Machine learning methods for constructing probabilistic Fermi-LAT catalogs

Classification of sources is one of the most important tasks in astronomy. Sources detected in one wavelength band, for example using gamma rays, may have several possible associations in other wavebands, or there may be no plausible association candidates. In this work we aim to determine the probabilistic classification of unassociated sources in the third Fermi Large Area Telescope (LAT) point source catalog (3FGL) and the fourth Fermi LAT data release 2 point source catalog (4FGL-DR2) using two classes - pulsars and active galactic nuclei (AGNs) - or three classes - pulsars, AGNs, and "OTHER" sources. We use several machine learning (ML) methods to determine a probabilistic classification of Fermi-LAT sources. We evaluate the dependence of results on the meta-parameters of the ML methods, such as the maximal depth of the trees in tree-based classification methods and the number of neurons in neural networks. We determine a probabilistic classification of both associated and unassociated sources in the 3FGL and 4FGL-DR2 catalogs. We cross-check the accuracy by comparing the predicted classes of unassociated sources in 3FGL with their associations in 4FGL-DR2 for cases where such associations exist. We find that in the two-class case it is important to correct for the presence of OTHER sources among the unassociated ones in order to realistically estimate the number of pulsars and AGNs. We find that the three-class classification, despite different types of sources in the OTHER class, has a similar performance as the two-class classification in terms of reliability diagrams and, at the same time, it does not require adjustment due to presence of the OTHER sources among the unassociated sources. We show an example of the use of the probabilistic catalogs for population studies, which include associated and unassociated sources.

==> SOM_VIZIER/3FGL_4FGL-DR2_Candidates_PSR <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  900 / width of table in bytes                        NAXIS2  =                   29 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                  112 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\3FGL_4FGL-DR2_Candi...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON_4FGL'          / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT_4FGL'          / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)_4FGL' / label for column 4                        TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)_4FGL' / label for column 5                    TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Pivot_Energy)_4FGL' / label for column 6                          TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'LP_Index_4FGL'      / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'Unc_LP_Index_4FGL'  / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'LP_beta_4FGL'       / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'LP_SigCurv_4FGL'    / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'ln(Variability_Index)_4FGL' / label for column 11                    TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR12_4FGL'          / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'HR23_4FGL'          / label for column 13                            TFORM13 = 'D       '           / format for column 13                           TTYPE14 = 'HR34_4FGL'          / label for column 14                            TFORM14 = 'D       '           / format for column 14                           TTYPE15 = 'HR45_4FGL'          / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'HR56_4FGL'          / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'HR67_4FGL'          / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'Category_4FGL'      / label for column 18                            TFORM18 = '4A      '           / format for column 18                           TTYPE19 = 'Class_4FGL'         / label for column 19                            TFORM19 = '4A      '           / format for column 19                           TTYPE20 = 'ASSOC_FGL'          / label for column 20                            TFORM20 = '17A     '           / format for column 20                           TTYPE21 = 'ASSOC_FHL'          / label for column 21                            TFORM21 = '17A     '           / format for column 21                           TTYPE22 = 'AGN_BDT_4FGL'       / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_BDT_STD_4FGL'   / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'PSR_BDT_4FGL'       / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_BDT_STD_4FGL'   / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'AGN_NN_4FGL'        / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'AGN_NN_STD_4FGL'    / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'PSR_NN_4FGL'        / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'PSR_NN_STD_4FGL'    / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_RF_4FGL'        / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'AGN_RF_STD_4FGL'    / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_RF_4FGL'        / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'PSR_RF_STD_4FGL'    / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'AGN_LR_4FGL'        / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_LR_STD_4FGL'    / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'PSR_LR_4FGL'        / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_LR_STD_4FGL'    / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'AGN_BDT_O_4FGL'     / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'AGN_BDT_STD_O_4FGL' / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'PSR_BDT_O_4FGL'     / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'PSR_BDT_STD_O_4FGL' / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'AGN_NN_O_4FGL'      / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'AGN_NN_STD_O_4FGL'  / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'PSR_NN_O_4FGL'      / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'PSR_NN_STD_O_4FGL'  / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'AGN_RF_O_4FGL'      / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'AGN_RF_STD_O_4FGL'  / label for column 47                            TFORM47 = 'D       '           / format for column 47                           TTYPE48 = 'PSR_RF_O_4FGL'      / label for column 48                            TFORM48 = 'D       '           / format for column 48                           TTYPE49 = 'PSR_RF_STD_O_4FGL'  / label for column 49                            TFORM49 = 'D       '           / format for column 49                           TTYPE50 = 'AGN_LR_O_4FGL'      / label for column 50                            TFORM50 = 'D       '           / format for column 50                           TTYPE51 = 'AGN_LR_STD_O_4FGL'  / label for column 51                            TFORM51 = 'D       '           / format for column 51                           TTYPE52 = 'PSR_LR_O_4FGL'      / label for column 52                            TFORM52 = 'D       '           / format for column 52                           TTYPE53 = 'PSR_LR_STD_O_4FGL'  / label for column 53                            TFORM53 = 'D       '           / format for column 53                           TTYPE54 = 'Flags_4FGL'         / label for column 54                            TFORM54 = 'I       '           / format for column 54                           TTYPE55 = 'Category_Prob_4FGL' / label for column 55                            TFORM55 = '3A      '           / format for column 55                           TTYPE56 = 'Source_Name_3FGL'   / label for column 56                            TFORM56 = '17A     '           / format for column 56                           TTYPE57 = 'GLON_3FGL'          / label for column 57                            TFORM57 = 'D       '           / format for column 57                           TTYPE58 = 'GLAT_3FGL'          / label for column 58                            TFORM58 = 'D       '           / format for column 58                           TTYPE59 = 'ln(Energy_Flux100)_3FGL' / label for column 59                       TFORM59 = 'D       '           / format for column 59                           TTYPE60 = 'ln(Unc_Energy_Flux100)_3FGL' / label for column 60                   TFORM60 = 'D       '           / format for column 60                           TTYPE61 = 'ln(Signif_Curve)_3FGL' / label for column 61                         TFORM61 = 'D       '           / format for column 61                           TTYPE62 = 'ln(Variability_Index)_3FGL' / label for column 62                    TFORM62 = 'D       '           / format for column 62                           TTYPE63 = '500MeV_Index_3FGL'  / label for column 63                            TFORM63 = 'D       '           / format for column 63                           TTYPE64 = 'HR12_3FGL'          / label for column 64                            TFORM64 = 'D       '           / format for column 64                           TTYPE65 = 'HR23_3FGL'          / label for column 65                            TFORM65 = 'D       '           / format for column 65                           TTYPE66 = 'HR34_3FGL'          / label for column 66                            TFORM66 = 'D       '           / format for column 66                           TTYPE67 = 'HR45_3FGL'          / label for column 67                            TFORM67 = 'D       '           / format for column 67                           TTYPE68 = 'Category_3FGL'      / label for column 68                            TFORM68 = '4A      '           / format for column 68                           TTYPE69 = 'CLASS_3FGL'         / label for column 69                            TFORM69 = '4A      '           / format for column 69                           TTYPE70 = 'Pivot_Energy'       / label for column 70                            TFORM70 = 'D       '           / format for column 70                           TTYPE71 = 'Spectrum_Type'      / label for column 71                            TFORM71 = '11A     '           / format for column 71                           TTYPE72 = 'Flags_3FGL'         / label for column 72                            TFORM72 = 'I       '           / format for column 72                           TTYPE73 = 'AGN_BDT_3FGL'       / label for column 73                            TFORM73 = 'D       '           / format for column 73                           TTYPE74 = 'AGN_BDT_STD_3FGL'   / label for column 74                            TFORM74 = 'D       '           / format for column 74                           TTYPE75 = 'PSR_BDT_3FGL'       / label for column 75                            TFORM75 = 'D       '           / format for column 75                           TTYPE76 = 'PSR_BDT_STD_3FGL'   / label for column 76                            TFORM76 = 'D       '           / format for column 76                           TTYPE77 = 'AGN_NN_3FGL'        / label for column 77                            TFORM77 = 'D       '           / format for column 77                           TTYPE78 = 'AGN_NN_STD_3FGL'    / label for column 78                            TFORM78 = 'D       '           / format for column 78                           TTYPE79 = 'PSR_NN_3FGL'        / label for column 79                            TFORM79 = 'D       '           / format for column 79                           TTYPE80 = 'PSR_NN_STD_3FGL'    / label for column 80                            TFORM80 = 'D       '           / format for column 80                           TTYPE81 = 'AGN_RF_3FGL'        / label for column 81                            TFORM81 = 'D       '           / format for column 81                           TTYPE82 = 'AGN_RF_STD_3FGL'    / label for column 82                            TFORM82 = 'D       '           / format for column 82                           TTYPE83 = 'PSR_RF_3FGL'        / label for column 83                            TFORM83 = 'D       '           / format for column 83                           TTYPE84 = 'PSR_RF_STD_3FGL'    / label for column 84                            TFORM84 = 'D       '           / format for column 84                           TTYPE85 = 'AGN_LR_3FGL'        / label for column 85                            TFORM85 = 'D       '           / format for column 85                           TTYPE86 = 'AGN_LR_STD_3FGL'    / label for column 86                            TFORM86 = 'D       '           / format for column 86                           TTYPE87 = 'PSR_LR_3FGL'        / label for column 87                            TFORM87 = 'D       '           / format for column 87                           TTYPE88 = 'PSR_LR_STD_3FGL'    / label for column 88                            TFORM88 = 'D       '           / format for column 88                           TTYPE89 = 'AGN_BDT_O_3FGL'     / label for column 89                            TFORM89 = 'D       '           / format for column 89                           TTYPE90 = 'AGN_BDT_STD_O_3FGL' / label for column 90                            TFORM90 = 'D       '           / format for column 90                           TTYPE91 = 'PSR_BDT_O_3FGL'     / label for column 91                            TFORM91 = 'D       '           / format for column 91                           TTYPE92 = 'PSR_BDT_STD_O_3FGL' / label for column 92                            TFORM92 = 'D       '           / format for column 92                           TTYPE93 = 'AGN_NN_O_3FGL'      / label for column 93                            TFORM93 = 'D       '           / format for column 93                           TTYPE94 = 'AGN_NN_STD_O_3FGL'  / label for column 94                            TFORM94 = 'D       '           / format for column 94                           TTYPE95 = 'PSR_NN_O_3FGL'      / label for column 95                            TFORM95 = 'D       '           / format for column 95                           TTYPE96 = 'PSR_NN_STD_O_3FGL'  / label for column 96                            TFORM96 = 'D       '           / format for column 96                           TTYPE97 = 'AGN_RF_O_3FGL'      / label for column 97                            TFORM97 = 'D       '           / format for column 97                           TTYPE98 = 'AGN_RF_STD_O_3FGL'  / label for column 98                            TFORM98 = 'D       '           / format for column 98                           TTYPE99 = 'PSR_RF_O_3FGL'      / label for column 99                            TFORM99 = 'D       '           / format for column 99                           TTYPE100= 'PSR_RF_STD_O_3FGL'  / label for column 100                           TFORM100= 'D       '           / format for column 100                          TTYPE101= 'AGN_LR_O_3FGL'      / label for column 101                           TFORM101= 'D       '           / format for column 101                          TTYPE102= 'AGN_LR_STD_O_3FGL'  / label for column 102                           TFORM102= 'D       '           / format for column 102                          TTYPE103= 'PSR_LR_O_3FGL'      / label for column 103                           TFORM103= 'D       '           / format for column 103                          TTYPE104= 'PSR_LR_STD_O_3FGL'  / label for column 104                           TFORM104= 'D       '           / format for column 104                          TTYPE105= 'Category_Prob_3FGL' / label for column 105                           TFORM105= '3A      '           / format for column 105                          TTYPE106= 'RAJ2000_Parkes'     / label for column 106                           TFORM106= 'D       '           / format for column 106                          TTYPE107= 'DEJ2000_Parkes'     / label for column 107                           TFORM107= 'D       '           / format for column 107                          TTYPE108= 'Tint    '           / label for column 108                           TFORM108= '19A     '           / format for column 108                          TTYPE109= 'DMmax   '           / label for column 109                           TFORM109= 'I       '           / format for column 109                          TNULL109=               -32768 / blank value for column 109                     TTYPE110= 'Separation_Parkes(arcsec)' / label for column 110                    TFORM110= 'D       '           / format for column 110                          TTYPE111= 'Category_Prob_3class_4FGL' / label for column 111                    TFORM111= '5A      '           / format for column 111                          TTYPE112= 'PSR_TOTAL_3class_4FGL' / label for column 112                        TFORM112= 'D       '           / format for column 112                          DATE-HDU= '2022-01-29T22:24:58' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             4FGL J0039.1+6257@^bB"ßÎ1?¿4GÛ5ñ)À9Xº'Gm}À;ß|ÊUú@oeÉÞZê?þ|óÁ-\Z?¾Í³ýsß?áú|2€…Ì@ Üa•FN@åÄè4Ý¿áP"G!ý¿Ú祖'R¿ÈëJw—¿äÉ"=—*¿ï6©Àd¿í ˆ JxIUNASNone3FGL J0039.3+6256?'{¶‹–?°Ý!	K>~?ïo§4YEc?°Ý!	K>~?¸h»Ê'¡?¶DVF ²Ä?ìòÿˆO´?¶DVF ²Ä?ªÁ˔wøˆ?›³ØEb?îSãFá»Ç?›³ØEb?³¦"î3?—ß?Xѧ?í‹-'f™‰?—ß?Xѧ?–_¿€ýÏ?¾A±Tù?ïM¢-3a?¾A±Tù?Œ‹Mo'@x?•7͟ü!?ïÒÊxð¾?•7͟ü!?‹}Yµ˜"?yÇ@EëFµ?ï'
™'N?yÇ@EëFµ?eßK4Ê¸?VG¤åî(?ïê ´ø½
?VG¤åî(PSR3FGL J0039.3+6256@^c {5*"?º$ª.gF‹À9köÔ{À;AŠ[@	.êú	q@;epÈ¿Á'áÙ¬âª?ïý°3Rׂ?yѦ p&ô¿áä³Ä›®¿ïÿü]šK,UNASNone@œ±¸ºÇËLogParabola?ÚѶZ¬…?ØÐÝJî?â—$÷R©½?ØÐÝJî?µjàÚ;n?ÁÀ…80'?íR½Öú"?ÁÀ…80'?µAâ֔ð¿?¥Û¯ÕÐi€?íWÃ¥£x?¥Û¯ÕÐi€?Á¬Îä˜à%?ª2™ÓwÍ?ë"ÌFÙÇ÷?ª2™ÓwÍ?Ðk}»ÜSl?×ɂ.Ã?çÊA"ÖJ?×ɂ.Ã?¡•N@¶Æª?´ý¡Uü?îæ«æÕ%?´ý¡Uü?µŠåœˆ~˜?­Õ€Êq§?íN£LSsM?­Õ€Êq§?œ,<~Huß?"E7"¶™?ïžzÁ?"E7"¶™PSRøø€øPSR@@ÞyÜe4FGL J0237.8+5238@aZsWæpãÀ®–ÃüC³À9ÅÛ_6Ç<À<VÁ1Ž…@Vá:B.?üèM&#€8?¾ÎG*`ý?㎧Þ*î@ tNrSÚs@T	|€"¿©q¬]f–¿Î÷çؖڿˮ)7'¿ã®T§!A™¿ïÓ4*…¿ïÛgNnUNASNone3FGL J0238.0+5237?¡z«ñú"?µý×÷AMO?îèU@›ø?µý×÷AMO?Á7†T~™?¾ÚeÍË`¢?ë²9jàZ?¾ÚeÍË`¢?²Uè>ïß?¢_# T?íµ^c/Ä?¢_# T?³P,¥:ç¦?–ñ•Ãœ?í•úktë?–ñ•Ãœ?—…K…™ÅT?½¾'CÜE2?ïCÕ£œ8?½¾'CÜE2?Ÿ÷+í…S?§DÇ«8?ïF ½5?§DÇ«8??–\½	$?wFÜ6çè›?HS¬?wFÜ6çè›?l®‹xðˆ?\±ÉD漞?ïãQð§aG?\±ÉD漞PSR3FGL J0238.0+5237@a[&ÉÀ¯"á¬WâÀ9.ŸÇ±À;pÌ؋Fð?ø4eø­P[@ËÊÒ÷‰9?ý;3L³Œà¿âo5ãå¿àà¼;bµ5¿ä&â涿ïÿéò§}UNASNone@oç ù	lLogParabola?Г6¤½ö+?ÉØò!<ˆ?ç¶d­¡ê?ÉØò!<ˆ?°%WOu·?Á-'ª'b?íûU:‡™?Á-'ª'b?ÞÝ­ùÓ
?³~ñéæì?à')rz?³~ñéæì?À"¦P[(?˜Å¢|«?ëÛký)6?˜Å¢|«?›:^íî|í?¤uÙÙ¢3¡?ï&-ÕDH?¤uÙÙ¢3¡?'å'Z ¥ö?¬ª¶–bT?ïhÓí8¹@?¬ª¶–bT?À<R6ÆY?ªB!é'ç±?ëðërNj?ªB!é'ç±?ˆTk÷{ËH?oÍu‡u8"?OøՃ?oÍu‡u8"PSRøø€øPSR@¨Æuù44FGL J0336.0+7502@`¢¦ YŸ@/DêÀ9ŸÏ!:ã+À<Y›0r@\kæ­ô?ütàaÕ.?¹	àÔk§™?ُ/Þ?@ 	ó蚈­@LŽ\¤œ?á%âØo˜¿ß¬übf§¿ÒQþ$ˆ x¿áQ"²ªØ¿í*ÎuCxü¿ïý/k'–GUNASNone3FGL J0336.1+7500?˜ÚÞÍ?¦	áDòÛý?ï?o¹mÁÇ?¦	áDòÛý?ÆjO1Ê?Àµ5'š2,?ê|ål3?Àµ5'š2,?º•³Ä?§³i-Óé?ì­_Üßiˆ?§³i-Óé?É#µãbv©?«'сítp?é·‡'bV?«'сítp?s¯*À=f? qeeX¡?ïØ¡ª'ÃÅ? qeeX¡?¢ðòÊLØ?¤A){Z†?îÐðӒ8Ò?¤A){Z†?"h£y?‡¯Ý×ÜË?ïdºçòíô?‡¯Ý×ÜË?Š¾ñTÜõ;?y´ŒþÅ\/?ï•:'K?y´ŒþÅ\/PSR3FGL J0336.1+7500@`£~=Á@/¼˜¢"ÕÀ9TîDì™À;—éŠrµ?øÀaÖá@,Ó¯*.?øûiÁƒ¿ÓiՒZ9¿Ü0®.ã(•¿ä׆‰ÇiŒ¿ë)'Jê‡UNASNone@e…8ï4×LogParabola?¤rU¤J˜B?³gõyí–l?î¸Ú¥ä'Ì?³gõyí–l?·GÖ2-"?ÂÈÖ	Ù¿ò?í9È-?ÂÈÖ	Ù¿ò?ÚùSg0;?·¬ŽÕ '?âƒVLgã?·¬ŽÕ '?Á¢ûW¤¬?š{Ã7%DÙ?ë—A*ÔÙ?š{Ã7%DÙ?o§TIƒ®­?p÷·–ã't?ïàX«ùÔ©?p÷·–ã't?Ÿªž«zR?²xà»#ÿz?ï«
Û%U?²xà»#ÿz?«эؙ?¡Êîeλå?îNÒçK±¸?¡Êîeλå?‡Lv–®Y?lšïý¢ÜO?ï¡ÂÎNà–?lšïý¢ÜOPSRøø€øPSR@É
vjYT4FGL J0426.5+5434@bÜ%Øם
@ûH
[À8VĘJåÀ;(&Ú@èÛ2k71@"÷Ãñ[ø?­€4¡Oùñ?Ùô/|ÅM}@$ãBؤ@ÿ:)Â?ÉÍ8¤û¿×ÄaÄ@6Q¿çÍù½ÆŸŒ¿í¦Á Hà¿ïü¨'Zà÷¿ì´¿ÍhUNASNone3FGL J0426.7+5437?v§ªbñe(?vÌfB¥§$?ïÒ°«GÛ¦?vÌfB¥§$?±Ôز¼³Ù?¯ÅÔ°8?íÅdéc±U?¯ÅÔ°8?͟ÛƒÚý?²¾¡Šm›~?蘉	A?²¾¡Šm›~?‡!ãMÄc?{GuÕ7\?ï‰ãxWL?{GuÕ7\?zJðÓ¸†?{S
ÕÕ?ïËjËG?{S
ÕÕ?†Kµhµª?ŒLW¹¨ÂQ?狀Ðå¤ú?ŒLW¹¨ÂQ?É#LÔL¦?³,ñì}'"?é·,ÊìÖ`?³,ñì}'"?žâÌ1mŽ?¢¶ÌŽÌq?ïÿ#	";?¢¶ÌŽÌqPSR3FGL J0426.7+5437@bÛ¾ ºK@ý¸ýâïNÀ8'£A¹ôÀ:¤UÖÌ*@PŠÇn¾ú@•†ø,L?ýæðõvO¿ÌÖùͶ¿ãUº¿ìÝõ›W_¿ïÿDUNASNone@Š Â\(öLogParabola?…§¬›˜¼?'ÞۃyÄ?ï©aMLäà?'ÞۃyÄ?¨ôjüqVå?À+Þ¾oo'?îp¹P¯B?À+Þ¾oo'?·¦¡±¬e?¦D×k#sÿ?í+É¡8
?¦D×k#sÿ?®.ÌrêN?Ñ‰Wԓ›?î8ìۋ?Ñ‰Wԓ›?ƒ^—jd?©ãϹ4k?ïÀùCð'?©ãϹ4k??ÒYÒÏÞ?ªç%)>Å?ï~mhcA?ªç%)>Å?–æŒۑ1?"Œs累¨?ïH˟¿è'?"Œs累¨?yX¢X"üT?f'§ìƒ;?ïÍN»,™ð?f'§ìƒ;PSRøø€øPSR@'…òPr'4FGL J0854.8-4504@p™¶Ãvö¿¡MŸßȖÌÀ8"Š'¾ÙÅÀ;H"ÅõB7@üíåKHÔ@
™#R ?´7¬"ž=?Ý/0ÓÊ@#ƒn—?üL+ín­Þ?êñ"¢A]î¿Û£iüóÜ¿Ê÷Ÿnc‹¿ã´k!a#±¿í]¶>•çÞ¿ïÿ³^¼£àUNASNone3FGL J0854.8-4503?:
äÁA•?4µŒ°À©¤?ïü¾£OŒ?4µŒ°À©¤?¯A¯ål?§Û‡Y2ó´?îåj¯?§Û‡Y2ó´?•*˼ž¯Ã?»l¼½?ïV©¡ñÏ2?»l¼½?…ꀗ'"?s5Að®0?ï¨Uý– ò?s5Að®0?NúUŒhÃ?9ÍwŠíœ?ïø}Á2 ?9ÍwŠíœ?€ýWQ†?'GŸß(y?ï¼ÞÒÖ?'GŸß(y?…ÐÌËEW?uôî>`ˆ?屮̛ñÛ?uôî>`ˆ?&¢ÏâÀW?ls"-?ïþ•Òî,¡?ls"-PSR3FGL J0854.8-4503@p™¤ü¤*í¿—tR§¬¬À856£*<À:ŠX;*xz?ýã!°SðB@qíVD?ù-Ö|ùÑ?Ó¬¨Üì!¿Ûɽ£º¿æ4È«ø8¿êc?Dä`'UNASNone@›ê5Y³Ð}LogParabola?yùÃÜ?™E'Çlƒ?ïÌyú±¦?™E'Çlƒ?§DJ1g/?¿qBn=?^+?¿qBn=?Ê?YZU?³!ُ@	?ép)©z?ë?³!ُ@	?¹–¹·¾•?•_D#¿z?ìÍ(É-\?•_D#¿z?XÀ'È•=¾?ZáNׄð?ï󟶂ø1?ZáNׄð?Œ¦
(.2È?ªí8ññÆî?ïgËQˆÅ?ªí8ññÆî?'qüäÅüt?'ê3±i8?ïlpõLü?'ê3±i8?Šà9ˆ
µ?tÔB‡ÅùÍ?ï"}Êþbé?tÔB‡ÅùÍPSRøø€øPSR@ExUñ4FGL J0933.8-6232@q£åÞÊmÀ¡2CI*ìÀ9þSW•éÀ<;<v¨Ô@­â˜»ù?ùï:µÞt?´=ÜÀ›ø*?æ&õ7O!¦@0M™gD²·?þ뮔¨n?ïçŸìš?¯GW™ˆ'?‡Æ¨½ÆA¿àµ¿äF¼¿îÚpžùÞ¿ïÿȽs"vUNASNone3FGL J0933.9-6232?^uz뭇h?c~·l§?ïðÅBg?c~·l§?±G<Ç´ô?°®™K!?í×fíäŽ?°®™K!?§dž{…Ñ?™Ú,åCï¢?î‡	¶&?™Ú,åCï¢?0ðax˜–ø?-1
}õÈ?ïýáô'ò?-1
}õÈ?l¨É#&K?mÏ°ÿÞ?ïãW6âY?mÏ°ÿÞ?…m~i¯Ÿ?‹¹[?ïªJfÿò?‹¹[?»Í&o¢ó?¨Æ#ñŒ?ì†[?R¢?¨Æ#ñŒ>µÔñùÈÖ>¾‡b8µ?ïÿýE‡ëê>¾‡b8µPSR3FGL J0933.9-6232@q£Âã>ÿÀ"`úÛÀ9¾ÙÅÔÀ;" ¨ìó´@jl(T@RãKζ¿×ÎR8œ¿Õ™éº]"_?°ïÒq¿á¤"gÑK¿îÊW…*ªVUNASNone@šÄ7éùrLogParabola?¿úH
¾b.?ɚ`E:?ì¶þH3º?ɚ`E:?®bWéïôú?Àk\fՙ?îځ7Åa?Àk\fՙ?±¶ò_¢_¸?£I:œäÕ?íÉ!´'0é?£I:œäÕ?³¼"$d­7?¢ÞP†>î´?íˆm›J/	?¢ÞP†>î´?ÃfQ°ö?ÓÙò÷Ñ)Ë?ë&xk»SÂ?ÓÙò÷Ñ)Ë?'™._šâr?¬d‹Ó"ã.?ïs6¥Ì?¬d‹Ó"ã.?®B1û^»?ª«­S[ö?îÜï§Å?ª«­S[ö?…)	鬺/?"z~©"Å`?ï«[ؐF×?"z~©"Å`PSR@aðDDDDDÀOCW›à$i60, 35s@JoÔj¹DÌPSR@í‹á94FGL J0953.6-1509@o|æÄŗN@=šO—íÇïÀ9Î,UÉ`1À<ˆ¢Ù´;Ü@"²U}5
?ú»	 :2+?ºžolIP?å(U{\˜@%%"1zÌ@9RIMü¸¿í<Lû[V?æžÞ&'d¿ÉMgfìs¿æ	s˜Ôx¿î"žã…uö¿ïûÌßÂðUNASNone3FGL J0953.7-1510?'¦ª¿ªÒ?¤Í5Öł?ïrʩ˯°?¤Í5Öł?ÅxܪæH?Á£×wÂüŒ?ê¡ÈÕFmù?Á£×wÂüŒ?º6¸Šä?¦ÝÍæ}M?ì¹(î¿C€?¦ÝÍæ}M?—»ýe?†ö.aã¯?ïCz''P?†ö.aã¯?—±œ'¢¿?¿…ÛTW¤?ïBsøÑZ?¿…ÛTW¤?¦ð:–ýþ‹?¥ý|KÒÚ?îüVt£7?¥ý|KÒÚ?•ßš.êÏ?FóùDK ?ïQ.CñX?FóùDK ?AÕ8…®ïí?8[W"»?ïûŠ±¹ï?8[W"»PSR3FGL J0953.7-1510@o~"t¼@=šÿ}úâÀ9Ý8§z¢À;ùõ3c¾?üR:Ð5@
É))D?Û«g𲸭?èz;ì{z¿ÎOo -¿çnS	½C¿ïÿ¬r†§œUNASNone@•á–R½<LogParabola?'ÍmEMž?šÅK@±?ï´ÊJø‡ø?šÅK@±?º:ߏ?ÄfӓæQX?ì¿X½ÜD?ÄfӓæQX?Á¦§çÎu?®Ëy?ë–V†c?®Ëy?³
%·D†_?š¯à¥>5?íž[I@ª"?š¯à¥>5?†èÍ "&?•êý j?ï¤\ËTt?•êý j?¥ö'W—?¸}צðo>?î® «f?¸}צðo>?ªêoÁSÔ?¡-övSY?îQ^:ä'?¡-övSY?wA\¸²úl?mA¹hØåÂ?ïÑ}FZ_û?mA¹hØåÂPSRøø€øPSR@®}KË4FGL J1026.2-5731@qÆ{²þÅm?–Òi!ŠFôÀ9éû±¼¦À;olŸe‹@Jê½£@|<âž4?Ŗ•BÇк?æ¢~ù˜@±À"š^»@qܗð÷ú¿Þž±{¸ˆ¿é֑Ýµñ¿¾Nx^
¢E¿ç±×JÕ¿í%óìÌG¿ïÿÚÁ,/´UNASNone3FGL J1026.2-5730?t¥
8øB?‰<ž˜'CÐ?ïÖµåÏ,?‰<ž˜'CÐ?¾kè9Z?µ­4Æ7/¸?ì2'øÝÕ?µ­4Æ7/¸?Ç
ÏðÝg?¬œ4µ†?ê<ŒȦ;?¬œ4µ†?ÂèûŽx ?£Í$"¢ó?ëEÁa×Ù?£Í$"¢ó?¢'Û·˜ª?Äø¿Cø'o?îݏD†u?Äø¿Cø'o?…­$<â?†°RR91?ï«åJhÌ?†°RR91?³ÈªÜÀ"?§"vnìÿ?íÆêé ?§"vnìÿ?s"w%ÜI¡?d^Sw=OŸ?ïØÙ¡	?d^Sw=OŸPSR3FGL J1026.2-5730@qÆM@$³>? µÐ±Þ´×À7Èn4'EÀ9þ¦-?ÿ¾‰öct@\è"ÿV?ü6ݲMD¬¿çƒ/NĀš¿Þ8I5[µ¿é®
Í{¦ó¿éE狏–UNASNone@œj'ø7´¢LogParabola?R¡ñÕ Ø?aT†œ?ïö¯9>/?aT†œ?¨qŠ£/æ?¿bÉ—á?îxçUö<ï?¿bÉ—á?ÈR¼v¤ˆF?±ýX:;«¡?éëPâVÝî?±ýX:;«¡?½'6]t?›ûuST•ø?ìM¼94\²?›ûuST•ø?Fvò•ók?FQŒG–Kº?ïúbX~‹?FQŒG–Kº?‹Øµ6£Ã#?ªèìøm7Ü?+@íÓ?ªèìøm7Ü?¸ÇðïÐz?°ýx^—ë?ìçâi?°ýx^—ë?<Ì-"tŠ?|Ø ϔ?ï‹ςoî?|Ø ϔPSRøø€øMIXED@L¦r	4FGL J1037.8-5810c@qàú;÷?Ï7äGè¡êÀ8¹Š>²Ã6À:_SUªL@±Ìp±m÷@z…\ '?ÁBL€·'?Òã%Ô¥ß@=B€®?ùÝ(¼Ü¿äÇÍ¿;Ò¿Û*«º®g1¿çƒhÀ2à}¿èeÌþJô¿ï›^?ÑQ¿ï¼~Æ.£UNASNone3FGL J1039.1-5809?ۘ<–r?Ô&ï+ÔD?â3áü´Æò?Ô&ï+ÔD?ÊAT‰D?Ãùiì`o?éyoªÝ¹¯?Ãùiì`o?ÜÖÊÍL'?¶2f[Ëû
?ᔚ™sÙì?¶2f[Ëû
?×'ÿÇK?²ö@¹¦T?ä|7Z?²ö@¹¦T?³gÉ-ê?µ"Ævëp†?í"ڇ?µ"Ævëp†?‹rwÑ#ÇÑ?…e£¹Q?ï'6 ÖíÁ?…e£¹Q?º¿'÷tý>?ªÊ;SçSy?ì¨
Á`X?ªÊ;SçSy?"H㳖z?wi'%"?ï®Üpü
ú?wi'%"4PSR3FGL J1039.1-5809@qã4¢3œ?ÖuÌ}ɯÀ8ÖmpEã9À:x‹îN?ùžv*úÕ@ü²ÎHøÂ?÷'\ÆÕfú?ï՘KÌîA¿à'ß\¶(4¿æ£% Bb¿ïÿá…ÓiUNASNone@žSoìVÕÐLogParabola?àzÙ®ë7? IõéçêÔ?ïxü)Æ? IõéçêÔ?«¢xelkc?¿pš0m?îEØy©9J?¿pš0m?Ç;f;?®{¤mˆ?ê99þ1&q?®{¤mˆ?ÃÏ{?ˆÎh?¢~ÇQÕä?ë!0Ìf?¢~ÇQÕä?nÀ¡æ-<Â?¢¯ñ¼ô§,?ïá?]ìwë?¢¯ñ¼ô§,?Nÿ•ÂŒ'?ªóÞš3t?ï'ÄÄr®?ªóÞš3t? Ôö`Ò&?˜Ñç÷Û?îò°šϽ?˜Ñç÷Û?•:õµƒ?'EݯÉî?ïS(œ'"?'EݯÉîPSRøø€øOTHER?ñ
ÞF	4FGL J1120.0-2204@qGà`þG™@B(ÂzÀ8Ígi›¥
À<ø¨ê@Þ}˜19´?üæ+ÈÛ¦"?«µÊ|»gu?Þäµ—&"@/êjP
@•'æxðW?ïùÙ?¡Ö¿¶UŒ_°zî¿Ý£¦ï¿è"kdÒè¿ïÿûbâMh¿ïæó{?UNASNone3FGL J1119.9-2204?'à,h"Z?›'.èi?ïpþœõæï?›'.èi?Ãý¤AN?ÀŠ¨˜˜›?ë:À–ï¬\?ÀŠ¨˜˜›?µh̺	}?¢í¨dž9?íRæ|ÿ¸?¢í¨dž9?ZPᨩ½`?VM׺–³?ïò׏Ϫ?VM׺–³?v‰×؍+?" Kêƒ#Þ?ïÒìPm":?" Kêƒ#Þ?¤âŒöù£?¤ÂÝÀÒýð?î±×?¹Ë¶?¤ÂÝÀÒýð?¡hµr©oï?˜õåþT·Æ?îét¨žoA?˜õåþT·Æ>ßp›X7>çt-C#?ïÿðH'2>çt-C#PSR3FGL J1119.9-2204@qGƒ[Õì@B†6`åÀ8Ώљ»(À;™tÆ{yô@$7÷E¨@Œgƒò¾N?ö
óxˆ'¿¥øV9]¿ß,âP–¿è Âb(‹¿ïÿê#¨YYUNASNone@ˆ½ª šª;LogParabola?…~8ð*'²?"SóÿÒ?ïªvOµ?"SóÿÒ?·–O
̳?Æ=Q±*?í
6u?Æ=Q±*?¾"vTTÊ?© 3Vbšü?ì-q>uug?© 3Vbšü?™ÓÓTºè*?€!l囸?ï1ae0ío?€!l囸?{Fq}˜?"Q菦r?ïÉsÊä%•?"Q菦r?¤>Vsqj:?º7‡ŸÝ£?»*ì?º7‡ŸÝ£?¼»?^Ì?¯pŏµ¢?ìhn'?¯pŏµ¢?c¤–®Êܜ?RÜYS³9?ïì[iCv³?RÜYS³9PSRøø€øPSR@ŸTOYý4FGL J1225.9+2951@g-©¨–h@Tñw[0À9'7 þ}IÀ<@̺XV@±È,)(Ã?üT¤MQÂ?·JRŸ	E#?Ú÷FóÚWÐ@"Ðàm"@±a5$$"?ï•¿,{3?ÌïÒ Ì=Ü¿ÑPLH­î»¿ÝΌ 6즿í]¨QÃA¿ïêo_‰RzUNASNone3FGL J1225.9+2953?y?ÂêÌK?¨—Û3¯êE?ï̀zJA?¨—Û3¯êE?Óm›ÓŸhª?ʩߕ"ê"?æI20K«?ʩߕ"ê"?·J\ȃ?¦bN.Û6|?í´fÆÕß?¦bN.Û6|?¤ÇuR›?'Ë,.â5?ˆªÖO?'Ë,.â5?r,kàý?šÙìÂvâ©?ïÛ§("ˆì?šÙìÂvâ©?¹§õÊ>t|?ÀA?VhR¶?ìËF¸1p?ÀA?VhR¶?§Çæ³þŸ®? 'íÝã?"À? 'íÝã?Wõ¥¯/í?PÓ;yoV÷?ïô-fj˜?PÓ;yoV÷PSR3FGL J1225.9+2953@g$ÞÊl @Tðñ¾ôœõÀ9wÒ4jkÀ;¨Öí·ÿ?úOó«³Í@>¥"8äù?óJCðð™?ÒïXæ© U¿àW¼ãÜÄù¿×UXÂ8õ¿ì'ŠyÉ£*UNASNone@›YW$tSLogParabola?®%Ê}»Ù?±d~‰yº!?î£^5â²?±d~‰yº!?ÜûìjKù(?ÒׂŠ€ÄX?á'	ÊÚl?ÒׂŠ€ÄX?Í¡\_ì§?²P€3❩?藨èûV?²P€3❩?ڋüt҇C?²i$žÕIœ?âºŖ¼^?²i$žÕIœ?‡.VsŒç?ŠbRŒh#m?ï£F¦$
ô?ŠbRŒh#m?ÑçEF䞃?ӕ‹"g•?ç]\°¾?ӕ‹"g•?ƶÛó?³1.4~‰^?ê{¹ÒI8ƒ?³1.4~‰^?¼Éí|ù-†?§)Ñ&ýœ?ìfÂP`ÚO?§)Ñ&ýœPSRøø€øPSR@0Êg™t4FGL J1306.3-6043@sþÚf@ÊصýÀ8kÚÜZ	À;"KâC@•û¯
t2?ü瀭9Š?±=z	3?ÝXʜpäo@)ð$p!Ñ@ú F˜7¿Á"Ê|æZ'¿¬\w`o聿Â1ÅIö™$¿ÝM1a!.¿êŸwßµ‡·¿î»úýŒ³,UNASNone3FGL J1306.4-60433FHL J1306.3-6042?wÑ{¾€n??­hþ!&?ïÐä\ò…??­hþ!&?¬C–³¯F3?¦·ïêååÃ?î;Ɣ›ÐM?¦·ïêååÃ?É5ڏO‹%?­¯ÓH»%s?鲉\,7?­¯ÓH»%s?†]¢Ò»??{ÍÆl|I?ï¥Ê‰ðc?{ÍÆl|I?bÁ‰eÚ{g?YLRԏ??ïí>vª£¥?YLRԏ??ˆ^'˜?€å¬:Ý«Õ?ïÁöïØaù?€å¬:Ý«Õ?§ß|êƹ·?£šÈ[¸ˆS?î'18…?£šÈ[¸ˆS?—ñÅÿ­?ƒÊ7š'?ïÿˁPÖ?ƒÊ7š'PSR3FGL J1306.4-6043@sKœ¶"Œ@±]''À8xÅ
»ªÀ:¶…F%~??ÿƒ>ùºì{@™;³4uS?õrjùs¿º¯&&bóÉ¿Ößë}ù¿àì6GöÊÞ¿ësiø¥²UNASNone@˜>Á$Ý/LogParabola?=L½"|Ã?Iðš¥Ç?ïüV|°Í	?Iðš¥Ç?£h¿èE?¿R$ÝQw?îÉwÑ|?¿R$ÝQw?µÕ™w
gB?¦èæ°d•?íELÑGŽh?¦èæ°d•? 2¶Q.rŽ?µ¸ï'QÒ?îüԛ•·?µ¸ï'QÒ?MErä'[Ç?Gz­	lš?ïø®£±$?Gz­	lš?‰½†b›v?ªñ'r·›?ï™	ç½òr?ªñ'r·›?‰Geys?‰]–Z¶4#?â‡bú?‰]–Z¶4#?lÈtR¢æ?[,B£õ…V?ïã7àlõ?[,B£õ…VPSRøø€øPSR@Ïv"Ø-d4FGL J1317.5-6316@s¿Ž`€¿áÄ* vmÀ8àÛÿo·HÀ;Ài;'@ÄØâ"Å@Ac?ÁÌm‰gÈ?â›êÂ+35@XÞô½²@Ì$'óÕ¿Ò¾0×@¿Ð¯ª}¬¿ËÈ©¼ýKñ¿æӉX=¿î<ƒß1i¿èPž¨øUNASNone3FGL J1317.6-6315?u[oÍ—?ƒ™ûÊ'_L?ïÕIý
hu?ƒ™ûÊ'_L?¹ïša}?±`Q	Ä
B?ìßBêÊ?±`Q	Ä
B?°‡?`'Zô?Ÿ™ã-›Ëv?íïû"?Ÿ™ã-›Ëv?ÀãhÝ0"•?¢=¾hP?ëÇ%ȳÚÛ?¢=¾hP?c–ëA"ŽZ? +7҄e¹?ïìi–ú? +7҄e¹?ƒa¿VÝx?…·‰™œI?ï²y§'ª?…·‰™œI?\öZw¶?|š" Ò7?ŒA?|š" Ò7?nÇPʒr?Z-»=šø?ïáo8Çò?Z-»=šøPSR3FGL J1317.6-6315@sñ¾ôœõ¿á3Ïp;ÑÀ8?M«"}©À:g"©GŒ‡?ù9í|o½'@a'ÇMµ?ûJ)©ò'>?ïêu^üº¦¿ã^,æ#é¿è&lX÷F¿îgùt±¾æUNASNone@œúÁ‰7KÇLogParabola?È0æIÍ?"\³ddç2?ïˆß?É¢)?"\³ddç2?²ãÝj۔?À•ßèTßù?í£œdªÎ?À•ßèTßù?Ë`áVnjò?°"Ë—D‹?é'ǪNÄ?°"Ë—D‹?Î7Ún~–?¨ÁÝ<P?èr8	d`Z?¨ÁÝ<P?Jq°¹Ÿ20?Màó?¬œ|?ïùc"Î(—?Màó?¬œ|?"(Z¡"?«#
MÕÒ®?ïf½*å©4?«#
MÕÒ®?š´}™µ}Ž?•eEhà?ï*\@ƒ?•eEhà?£lrº˜Ô?Žên¾ç–Y?îÉ6ù¢?Žên¾ç–YPSRøø€øMIXED@™""ó4FGL J1329.9-6108@s9"t¼?ö&Ks›ÙÀ9œ§ktÀ;^iŸÖÊ}@Ù؅½™©?ÿà,%!øx?½ø+஁?ÙÒüÇf[@710ýÏ@®€™B†¸?í½ÚÁ'ï¿Õ™0þz™Ï¿Ó¥!ÂÈg¿ã¿YG¿í-¢Ðzw¿è@<›'Á^UNASNone3FGL J1329.8-6109?œÜšCdc?©£$:z'Ü?ï-ò›W?©£$:z'Ü?ÀëU³Þ?µl~+ëE?ëÅ9ª"}?µl~+ëE?Äd^º)?­`K…"ž?êæèyÑ}6?­`K…"ž?ÖÿÕsöƒ?²-0'ÝH#?ä€F¾x?²-0'ÝH#?xtØK[u(?›ŽÂé?ïÏOf‰f?›ŽÂé?… úVµÓ¾?ˆ#åÍ?ï©|À¥'?ˆ#åÍ?š])j¡M\?'çÝIq¹?ï-´ªõ•?'çÝIq¹?™Å
ږáo?ƒÄEÃo]?ï1בT"D?ƒÄEÃo]PSR3FGL J1329.8-6109@s8ҝÇ%Ä?õÕ`IôÀ8ÔG'‡|À:€ŠÔÚ¸?øBw÷]o@Åßó›?÷pµµ.£¿Gctö/¿ÝÓÙ"à¿âõ‡›D¿î¼P3°AãUNASNone@˜¸²a|ÚLogParabola?™Âjú'?¡æ1é|?ï1ïä~ð ?¡æ1é|?É'SØwÙ?Âü[/Ñ~ã?鹫	â
?Âü[/Ñ~ã?ÓªY'9ö=?²§ÎߣH'?æ*Ó6ãá?²§ÎߣH'?ܐç'…Ä¿?«ii»…|¬?᷌l= ?«ii»…|¬?d1Æ|s¿{?f'¤3äš?ïëÎ9€Ì'?f'¤3äš?žsíáMž?­Ðå#DxŒ?ï`—U­Ã?­Ðå#DxŒ?­*üñÂJt?¢P%^î©À?î-P0Öé?¢P%^î©À?ºZ:…
_? ´ÃðÉðé?ì´¸¾o^T? ´ÃðÉðéPSRøø€øMIXED@ÀÄ*ç¶4FGL J1358.3-6026@sqŸÝëÙ?õƖ^¤ÑÀ8"n°'-À:d>XˆW@x=û»ù@‰¤Y=?±XR&"g¦?ÑyYˆ1'@@@&`½?ÿF
ñ/W±?îöø_LÁ¥¿Óîtý­ë5¿ãKíÿ¢b¿èÉf@¿ëÓß ¹ôX¿é3€`°UNASNone3FGL J1358.5-6025?³oøï1?ÀY(í½'?íò¸âŠ?ÀY(í½'?¶‹¬n©?°'†wR§?í.Š|›1?°'†wR§?˶Ô?³ñÞ§†:n?é~Šýýû?³ñÞ§†:n?´NTʐ:(?›d…'×q?ív5fò°ë?›d…'×q?k žOœ¯}?'‡öâ}–·?ïä_aÔ@?'‡öâ}–·?'†¹ÿ}ìš?"ù1›̶?ïµåh&?"ù1›̶?‹œÅ$g)?Îù½­®?ëòh#?Îù½­®?S(s"_"?Eïó&?ïökÆfp?Eïó&PSR3FGL J1358.5-6025@sr	ԕ+?õè|4gÀ7䐴Ê!À:Sýå¶?ûI"dvL8@Éf<J7@Çþ†Ù#¿ÒVƒ¾Õ­
¿ä˜Ñ1$T¿è'&›É¿ï-9†ßW¿UNASNone@‰Ñë…¸LogParabola?ƒÝS,;d?'p÷zU1?ﰊ³×?'p÷zU1?©¤¥a/6?ÀæažU–?îeµª$ü?ÀæažU–?Æ1ƃ::?¯•GñÎgk?ês¹Ž_1q?¯•GñÎgk?Áö,Èò?›Ó¥ëÕ4?ë'tÍÃ~?›Ó¥ëÕ4?@'«Ã­f?C~ö>`Ķ?ïû۔Õ~f?C~ö>`Ķ?ç3eë?ªç©‹¼þ?ï‹Äc
«?ªç©‹¼þ?•¿Ñk>›?"ok¡"?ïRwy^;?"ok¡"?''U˜1?zÐl¾i¬?ïvÇUD¸?zÐl¾i¬PSRøø€øMIXED@ô5@\D,4FGL J1405.1-6119@szOß;d?Ò&Ÿ;š
À7€®I#À9iÞÎW@	¿Bu›c@PŠ"Ràx?±M
NóA?Ñ(6À[zO@"µz»ˆ?öŒ¯˜ß_w?·Ë¼V‡÷¿×ˆï]J¿æ«"zuè¿éç.þL²¿ë'®/RÓâ¿åï@4£UNASNone3FGL J1405.4-61193FHL J1405.1-6118?Š'îiQ=º?ªmò*'?ï—`F'´É?ªmò*'?¯þ²Û±'t?¨_) ÙÁ?îÒ
î?¨_) ÙÁ?ϱ\#Ax›?¶gdw<¼8?è¨÷/¡Ù?¶gdw<¼8?qGŸ·üí?cäÙ>»I?ïÝÅpÀ?cäÙ>»I?x0fn?­9äBÙE?ïϟÍ1Ãê?­9äBÙE?€ìyÜ·[?'áuýáÙ?ï¼Nä.‹?'áuýáÙ?¯#ï,úÞ#?£ùœã?î
Á
Õ>?£ùœã>éŒCLô‹>æó­°0ux?ïÿæsÖ«7>æó­°0uxPSR3FGL J1405.4-6119@s{!Bp?ҕa¼­žÀ7Ґ[,À9Ëp£×
=?ÿñ´â@BüŒX'?þ_ÛÛ£
¿Ó‹
9ÏYš¿ä]ï֫⋿çvº 5¦;¿ç"vµû
^UNASNone@ ÏRn—PLogParabola?tžI{!õû?z~K,Ÿ«b?ïÖÃlë"?z~K,Ÿ«b?¤È'~¼+?¿|ÃÏ<¨?î³~æ¡~?¿|ÃÏ<¨?Ð)¿*ä°?²ð 1Pi?çë tꍨ?²ð 1Pi?°…ƒJîRé?'fûén8Û?íïO–k;ã?'fûén8Û?sîyˆœ?":û$ã2?ïØ#Ó§?":û$ã2?ŠŠ®îó?ªíƒ…öh?ï•×ÅE¼D?ªíƒ…öh?Ò€eô")?¹°vø&d?æþ?ͽë?¹°vø&d?~œ[?nw´i¿?ïÃÞÇK-¦?nw´i¿PSRøø€øMIXED@Y\V˜T4FGL J1539.4-3323@u,šÔ,<Ÿ@1ˆ5ĊßÀ9(¼QT†jÀ<süQ×@ô$ª"N?øÿ0F祥?´þï3Ôî¯?ä']<ñøÖ@+‡_•'Í@æCÍ_CÝ¿ÓVºÂG¹?ïùgÁf?¾"–}/€¡¿ß';#l–¬¿íH>]2àþ¿ïéŸ
ç»UNASNone3FGL J1539.2-3324?a}íæ?qûðŽanè?ïî'äMj?qûðŽanè?³Â›é?²"*¥¯¢Q?퇽ª!@?²"*¥¯¢Q?°SÒZUa?ŸÕ/	}?íõ…´p›°?ŸÕ/	}?d+CŽ>Ùo?\b±í?ïëÔ¼|¿ç?\b±í?]IïT7—ø?TøkžKŒ?ïñ[S$"?TøkžKŒ?ŽZ©[èåÛ?•¯lã¯Ç–?Zg!?•¯lã¯Ç–?¼ÿ;+q•;?©PVòq?ì`š'ÍY?©PVòq>üq®
ò>ûFÁ•ÒçÐ?ïÿÇéÓv>ûFÁ•ÒçÐPSR3FGL J1539.2-3324@u,%ãS÷Ï@1ˆÁDŽPÀ9.èŒEôÀ;š^x[[p@(Ò·rrŽ@;«Ò(+¿ó…¦÷ú"?ïþ°Q/â?ç¡eº]Î+¿Ü>S"ø䔿í‰ÕB€òÈUNASNone@¢›~ùÛ"ÑLogParabola?Éóožs?Òº¦˜õH±?éƒ>;$c?Òº¦˜õH±?¶Ê榸ï?Ãd£ǜâ?í&£=á?Ãd£ǜâ?»
ÛY?¨'5¶R?ìœÜü^¤•?¨'5¶R?¬<ÍYÈDé? ëö*
¸?î<3*,ò? ëö*
¸?ÊgÊ\¸›E?Öüu™+¬ù?éf
hÑÙ/?Öüu™+¬ù?¥¹UTù?·ƒœ×¤‡­?î¤j¯¤p?·ƒœ×¤‡­?¼'ó¨Èzq?±@|Á`vÒ?ì{Šæð²?±@|Á`vÒ?† ¬|ƒ?‰ÝpEþ¶?ï§~@O"?‰ÝpEþ¶PSR@mZÀ@¶Ó m:60, 15, 52,60
@N>ï='gjPSR@_m»36(4FGL J1653.2-4349@u\Ù@x–?­‹ÛàùïÀ7œƒujæ(À9Žß‰gó.@@éTA÷@=¼>	P?¹{'G•Á?Ҁ¿®Xë@´û'Ã@æb I?ïþ'ÍzÈ?ãm¬átú~¿å—˜mI¯v¿çךÈÙ"¿ì'†!퐒¿ïÿ踻ÐUNASNone3FGL J1652.8-4351?ªTÎe2œ¦?¼a'Ú?îZ³ÈS?¼a'Ú?¸Ú¹³59,?²ºÆÈ5jC?ìä¨Éb_?²ºÆÈ5jC?ŬsK¸?±Á[³z®V?ê"ÿã>m?±Á[³z®V?Ÿ'q—™z•?ŒïSGkG£?ïìs'·K?ŒïSGkG£?¥°ºKڍÄ?Á…¹çn0?î¤ôZýžô?Á…¹çn0?‡ý«ž,?Žqw_´¥Ì?÷?Žqw_´¥Ì?¢¯ÿb{i;?˜NEH¹¡/?îÕ	æÜ?˜NEH¹¡/?3è§'—Z?,ÊK?s"?ïý'ë4õ^?,ÊK?s"PSR3FGL J1652.8-4351@u[¼w¯d?·‹Y:À8]–
˜à6À:_yv
£W?úÎMÖL¨O@«}ůÞ?Õ	u…ÏI?ïÿî]ýG¿²§3zʯ8¿äòç
2*¿ë¡ ۆ'ÆUNASNone@¡ë•Y³Ð}LogParabola?±-'ú"?ÁK¡>(¯¢?íݺM÷¸;?ÁK¡>(¯¢?ֆ
úÙ>d?Í%'»±œp?ä¼ù"`Î?Í%'»±œp?ËËÖá	?±Øs›™~5?é;
 
G¾?±Øs›™~5?Ý!ý˜i[?¸Kg'Ç"?áo3ËxS?¸Kg'Ç"?‰Àõ-](?±Š2ڄ¼?ï˜ü+<ÍC?±Š2ڄ¼?·F]YzÚ7?¿u.O;?í4Tùà	?¿u.O;?¯¡3 PÈé?ªPæºn,W?îìÎpQ?ªPæºn,W?À¬	£EÀ?±)ùr¤
¬?ëÔý»W.?±)ùr¤
¬PSRøø€øMIXED@*Œù<4FGL J1730.4-0359@3¼î¿eÛý@/ý™gD²·À9¡ƒJ¢»À<	²öañ@ûŸZMÔI?þ´zuçãª?À_©]ÜÕ?áp'S­Q@B¸A$~?ô˜0m±v¿ï´qV"q?ïÿÔač¿Ãݨè)b¿æ¶ã¡¥¯¿ì´/GhG¿ïÿûÞ]BüUNASNone3FGL J1730.6-0357?Š`ôùØ?›ò¡3)_?ï—â|Xãh?›ò¡3)_?±·ñŸ?³Ed½›Œ?íÉ,&_Ì?³Ed½›Œ?ºUChài7?¥Ä[~ÊÄ?ìµW'ãòÙ?¥Ä[~ÊÄ?"Ü.qi??|Ùÿ´ÔÔ?ïazö?|Ùÿ´ÔÔ?®­ôÑ?¯1tr;Þ]?ï¹G•'"?¯1tr;Þ]?Š‰Hv?•»À*À"?Ûéw?•»À*À"?¥õç[?~C²ÑˆÒ,?ïh(™k?~C²ÑˆÒ,?E'ÄààL?:|®_g>?ïú›Nûe¼?:|®_g>PSR3FGL J1730.6-0357@3ͽ@gÏ@/în"ŠzÀ9Ä斢nTÀ;gæ…·?øðMÈà¯@3·«þK?ߣK¥¤¿Ú–ú©T?¶k\€š«N¿â_lµñû¿îT'BÙiUNASNone@™)ó¶E¡ËLogParabola?"8ˆ@	ì?¦O.mO‹?ï¯ö™À?¦O.mO‹?¸1VDfÂ?ÄkTHù?ìùÕ7:ºø?ÄkTHù?Êú8‹¦?´mêj÷­'?éA[ñÝ`?´mêj÷­'?ÃÍÏ\?ªà')ñh?ë>¿ùL)?ªà')ñh?€_qˆ?§¢–ž`ªo?テ'…ø?§¢–ž`ªo?eÄ¢SHõ?¶†¬L¼«ž?ïÑÚíe¸?¶†¬L¼«ž?°ÿ[¹eò?¢'­™Ö«H?íý {Ò?¢'­™Ö«H?ŽG—0m7?u)°"&+?ï†á£Ô?u)°"&+PSRøø€øPSR@þÀ-"GW4FGL J1740.7-2640?õ³é÷þ¾@ÕinX£/À9¨‰ò\©NÀ;L'݃Ô@ð¿Îâ{¶@;½Ep?Ñú"å$²g?å7]ú14@‰0«½?þûþ0Gœ?ï«íßl¿⎧Þ*î¿Ø ­ŸŠõ<¿æŠw½¦¿¿ïÑdBSb¿ïäó¿ÕÃkUNASNone3FGL J1740.5-2642?ÍÈkx7ãá?ÈÿA<	P?èå!ò?ÈÿA<	P?ºî!h&ý<?¾(QdÃñS?ì¢;Òû X?¾(QdÃñS?Õ:Q¨œÊY?²f¤²ºB?åb×+±šÓ?²f¤²ºB?¾¸P`bÝ? ;C¹BuS?ì(õóó¾d? ;C¹BuS?Â~µÙ|nÍ?Çÿ¥Fú:?ë`R‰ äM?Çÿ¥Fú:?"ºÄD©?˜ðÁæÃ,¶?ﯥ	Õ?˜ðÁæÃ,¶?»Ø"ôÕ2?¥ñª8–8?ìŽDû¡eZ?¥ñª8–8?{ßÚHÈà?iúéeíÄ6?ïÈ@K¨'¯?iúéeíÄ6PSR3FGL J1740.5-2642?ôÞ i—sO@û¿¼CÎÀ8ÏËRyI˜À:µ½Ñb^?øºQO}ì•@ìG'd?ô4đ?¿±ïGºU†,¿àìi9i¿æIæ¯æ¦×¿ïe­¾ê‹úUNASNone@˜WLL˜_LogParabola?X÷°cå¢?mg6?Ä
?ïó"|Q	]?mg6?Ä
?´úõÏÜhú?ÅKs2&Ä?í`¡Eèö?ÅKs2&Ä?ÊøŸA+÷Þ?®âe{´ö$?éAØ/µ?®âe{´ö$?Áä§rRáW?¢_ò~Ä?ë†Ö#kGª?¢_ò~Ä?Ob`ºƒ]¾?`¼^ÐMëZ?ïø'h§¼?`¼^ÐMëZ?Ÿî&Oj?¾oªaµI?ïn¿È¥?¾oªaµI?¿i7«VÊ+?¯"œZ@û?ìÙ
•&»?¯"œZ@û?Œ±"ýOp?vŠƒÑ¯(X?ï;tA½²?vŠƒÑ¯(XPSRøø€øOTHER@Ÿ"ÈìØ4FGL J1808.4-3358@v`º^5?}ÀæØnÁ~»À9…ëOnÓÀ;ÙJr'@pޚՃÖ@Íþu¼D¿?ÀN¢dïBî?éV؉™qV@#4h‡¨ÖM@ð™/¼[;?ïõÞs¾=¾?Èz Ûmé¿àEæÉÎË¿êøToÃÝ:¿ïÿ¥'(^?îK]@ÍЃUNASNone3FGL J1808.3-3357?Œè›…8*í?²•M#©?ïŒ]'´%•?²•M#©?ÀhýÍÿ/~?¼Â&€I?ëåÀŒ€4 ?¼Â&€I?Çs4L…6?°[g¯¼œ?ê?£2ìÞ²?°[g¯¼œ?¥˜Q×p•?•1>Ô`›Ê?î¦zâŽ÷?•1>Ô`›Ê?§5EÛL.'?Æ.O&aq=?¢/À7?Æ.O&aq=?›™ùµ3?£È‡°Èf4?ï#07;'¸?£È‡°Èf4?¬%WGCô?©üŸ§3½?î=®Ú§¡?©üŸ§3½?;Ô$eñ€?4%	@?ïü…{nO-?4%	@PSR3FGL J1808.3-3357@v`÷<ÉÀÚ\¢˜EÝÀ9w;ØbçÀ;DŸqIï7?ø
.j€@oÅz¤6?ôž9ŒÈZ¿Ö¾l$žù^¿Û‹ÿÅ*¿çVïó9ëV¿î°¸ë!)NUNASNone@•¢Â©"áLogParabola?ªч!?°È§\–õ?î^Ÿ2¾KÞ?°È§\–õ?ËK!7CtZ?ÆLÜ|˜,?é-7²/"é?ÆLÜ|˜,?ÔÌä¨>U¯?´¤Hº¨	?噍«àÕ)?´¤Hº¨	?ÙTeÖQ8Š?±fi%?ãUÍ×c»?±fi%?~ñ›¥˜Är?Š×ÎsÅû?ïÂÈÁ-?Š×ÎsÅû?›ä¨æ²‰Ò?°B<Ð}ÌÙ?ï Ú¸ó§?°B<Ð}ÌÙ?²jê¯ÕÍ?¤#êé3?í²¢ª†Ö?¤#êé3?¬¾ñWpª7?››éZ@ ?î4êÍ­Œ?››éZ@ PSR@qwwwwwÀ@÷¤úO¤ú56, 60, 60,60ó@Yê™ì
T:PSR@xDÊN1*4FGL J1823.3-1340@1˜³€Ëlz¿½kW½VÀ7d_4Bý¬À9Ðè±.á•@VIã£Ô@0k_Êjó?¬b¡œ»­?ÏWŠý@Áæ??öÍþîˆx?êÔ½‡	Ÿ?Ó¸GD7<'¿à¤¸F-
û¿ã!½êÜ­¿ê
Ä
áj¿í¼ã`7"VUNASNone3FGL J1823.2-13393FHL J1823.3-1339?•mû8Ά>?°d½LÓ?ïT&9‹Î?°d½LÓ?œ@ÍÍHÑ?¡+jCij?ïù'À¡	?¡+jCij?ÅtÀlþAJ?°õ@2,õm?ê¢ÏäÀo­?°õ@2,õm?xZ1xjÄH?e%"Ÿ–×?ïÏKjÇ?e%"Ÿ–×?€j©èc?±œòùo?ï¾U["¾Ÿ?±œòùo?n}UÅG0
?~UóÍÓ?ïႪ|@?~UóÍÓ?™žÿ¿P?˜*%²_ ?ï3ôE&?˜*%²_ ?·¿ðý+?&¢ÐÀ¡·?ïÿGJKˆ?&¢ÐÀ¡·PSR3FGL J1823.2-1339@1š¥ç…µ·¿¸€,5=$À7jf¦'GÀ9R[Æ?ùJšèùÿ
@䓳%±À?ýwã:"¿Ø`ð"¶—¿à¿Ÿ×eü¿ä5†‡8¿è"†¸ýsDUNASNone@™?!aä÷fLogParabola?©ÄÖlva?µzóÅ)ØP?îc²™¾Ú?µzóÅ)ØP?±ë۞¶^Ø?º¿™¯$Vˆ?í"Œ
·E?º¿™¯$Vˆ?Óͽ¼ÓIW?µ
"?æ!!–[T?µ
"?Ô>Þq(Ðó?ªjd!¡?åàÇk—†?ªjd!¡?€TI,À"?‰ùJW‡¾?ᆴێöA?‰ùJW‡¾?SϟŠÖP?¦,!s§žh?ï}a'Úmþ?¦,!s§žh?Ñ1(E»Ã?µÕUæÊ ‹?çg~ëÝ"?µÕUæÊ ‹?±zÊIÛ?"ÌÐ&R?íÜ_0´u5?"ÌÐ&RPSRøø€øMIXED@}!Ç4FGL J1831.6-0223c@<ŠÙ'N"£@
orÖٖÀ8® HtäÀ:b4"F{å@~og–è@ñm*¥Åø?ÆèÐ#ˆã?ϏŠâq¤³@?òÿf}
?ù~‹=á7?ïh
?®–¬?ã"Ág	¿ã^PþJHN¿ævéki¦¿ê±ôÆ/¿ï÷™^á6çUNASNone3FGL J1831.7-0230?Ѧœå‡€?ÐZL¹"h?ç,±<z@?ÐZL¹"h?Ã
:Α?–ìãe?ë<±xL[½?–ìãe?ÚA&ç܃à?·þ‡î)‹?âßlŒ¾?·þ‡î)‹?Ë!Ws-t?­æaÞÂB°?é7ª8£4£?­æaÞÂB°? Çô³· ??¡âxñÞs ?îó€´à
Ü?¡âxñÞs ?"X?˜X5?¢‹dæ7?ïe>Í~Î?¢‹dæ7?ÄKšŒw‹ì?°Çs ?êí\â?°Çs ?ã¹['"?€C¹· ˜?ï‰øqÔò?€C¹· ˜ PSR3FGL J1831.7-0230@<u^á6ç@	Ó˜K$ÂÀ7àùx&'KÀ9ÆõkQ‡²?öÉLÌKž@»PÒ@´þh{>¿ç"=ý;ª{¿èóAç½$¿êF$mƒÍ;¿èõM¤E£UNASNone@Ô1²•êLogParabola?†$‰HÔà?ªo`â£6?ï§ÏmÍ=?ªo`â£6?®/šBÿš?½a~ª?î[ÂQ&?½a~ª?ÐÚ1GSYL?´IïÚ¯O?ç'ç\VSZ?´IïÚ¯O?Íâ‹›ee?ªŽ¾ƒº³e?è‡]8Y&§?ªŽ¾ƒº³e?p<òbRA?'Á'Ô¡¦…?ï߆sµ?'Á'Ô¡¦…?üc'CV?«]'°&¬p?ï€q÷'ó?«]'°&¬p?Ì»ž!5&?³‰ð`ÿ?èÑ>Xw²¶?³‰ð`ÿ?šÄ4LL?ˆÍt^îð0?ï/YÞ(ûÞ?ˆÍt^îð0PSRøø€øOTHER?ý¡YÆ3Ä4FGL J1843.7-0326@<þŒ&?¹hšY³À8/r&À9|_æ¤í@W­»åt@ºd<Àz¯?欂ªiËv?¾²pK˜?ûV'QúŸ?ð•˜/âè¿mÜ	‰IGû¿Í—Ðk½¾<¿äÉh^Ž*Ñ¿éªÃø贊¿íþVèD!˜?ÜõÇb)ÀÄUNASNone3FGL J1843.7-0322?Óˊ=Â>?Õ×ÑÁ0ë?æ:áà¸?Õ×ÑÁ0ë?ÐùÓÙ?ÌôÇ+'íí?çƒ|–uð?ÌôÇ+'íí?ÛäòÇÌ÷"?¶Ðbîº?â
†œ">?¶Ðbîº?Ûj""B[U?»)ÒGœ2?âJ¶nÞÒU?»)ÒGœ2?Ø!y}x?Ø-K…ä?ãðowÃAD?Ø-K…ä?"";•l?¤‹YÌ
kO?ïca'óæu?¤‹YÌ
kO?Ù-¤þ҃?¿–ÀÕD?ãwé-€–¾?¿–ÀÕD?'Ê+ëgØÜ?ˆKšM­D?ïi® Íü‰?ˆKšM­DPSR3FGL J1843.7-0322@=çáüú?ƍ¥šƒÏXÀ7ªñÀ9À¨á59ž@"Ùz/F@'Ý<Ü@CÕÖᣟ¿Ü;š<#>¿çòµ0Æ=ß¿êmIçՑ¿ïÿAHl"UNASNone@ÙÁü2LogParabola?¥›èVm?±ÏgbK	û?î¯6P÷y?±ÏgbK	û?–µçíŠi?¶H¤õÈb"?ïJP—X]?¶H¤õÈb"?Î KmfŒ?²H<<¶?èwí$¹¦]?²H<<¶?µƒÆ¤̧?–—±«ìÔë?íO‡+¥A»?–—±«ìÔë?¬ÿ¸4ðª?¸­5ZdVj?î0|ç\E?¸­5ZdVj?ƒÝ´¼·K?§w±'è~ä?ﰉ-ÌÓ?§w±'è~ä?Рºty­?µž}š°Q?篢ÅðÃ*?µž}š°Q?GGšÑۈ?{Z^oõÏÜ?ïŠâáPb?{Z^oõÏÜPSRøø€øOTHER?ݓi 2ê4FGL J1858.0+0354@B•Êl <K?Óу€R ·À7òŸûÆÀ9ß:Q4¥ú@*ÜGéùƒ@@öÍ0 ?º¾Ä÷@hÑ?܆—^Uö­@!
hn~bÜ@dªõ°7¿ç¿sFS¡¿¥ÁÍBC‹¿à'" ÔÇ¿ê_@z¿îJ}ғ¶¿ïðÌö%ŒUNASNone3FGL J1857.9+0355?²ô\_†¶?Á3©©öÍÁ?í½!t«é?Á3©©öÍÁ? T¥!KÏî?¢kTMA?îúµ®"<Á?¢kTMA?´›–FÜeû?¥t1ïÖ?íl7i+p?¥t1ïÖ?£Äý
²U?'ÌÁm'z?îÿø[?'ÌÁm'z?qÍàGÑÄd?§ª<NñÇÜ?ïÜd?£6¯?§ª<NñÇÜ?qª	q¢hx?€/Ë{:GG?ïÜ«íY4O?€/Ë{:GG?ˆ«·³í4?zpfý]‹é?ïQ!ZÛ?zpfý]‹é?8êd¥Š]*?0ð6‹Ÿ­?ïüâ³Wʆ?0ð6‹Ÿ­PSR3FGL J1857.9+0355@B•Î|Ð57?Õñ÷(ÀéjÀ87¸Óñ"À9Ü7i"ÙI?ûMFˆï@Cˆ?ÿõ?úÆ3
nmò?ïšÞw3#¿á•¿Ù8/¿êºÜÓç.‰¿è"HÒõ UNASNone@šy¥`A‰7LogParabola?ª"(jAà?¹èX¯?î]Ý~©[â?¹èX¯?À¨…‹«Ön?Ã9׌eÌ?ëÕޝ
d?Ã9׌eÌ?ьy	Ô?´<yá*â?ç9Ã{rð–?´<yá*â?ÙÖZh	m?²hRFŽ?ãÒËû|Ê?²hRFŽ?lfDãÍÛ?x'Ìü¡ì?ïãæ™ÒyŠ?x'Ìü¡ì?¤•53xp?±p;œŽ@ ?¬ñ»?±p;œŽ@ ?Éò5–S­Á?µi1%·º?éƒršk?µi1%·º?½zïaÕ?«Žbâ"t?ìP¯ÂÐ?«Žbâ"tPSRøø€øMIXED@¹°çO@@4FGL J1900.4+0339@BœÉÙÓE¿ÕÕ° CÂMÀ8'_3l>À9í¦Ý@ø.åƘÖ@¢=ú	F?¼üÛ2k71?Õ,áàZH@IS.Ô)@TöÂ>©^?ïÿý{ÁA¿ÕbàõΤ¿ãCàµ7¿é)Ùîm¿ío¶;ÏÆ¿ïýŸÝÂUNASNone3FGL J1900.8+0337?µ:U"ŠÌ?À¥*.Û=\?íX¿U&3W?À¥*.Û=\?¨°
V<š?©ž˜›'¤?îtÿZW~0?©ž˜›'¤?À°e sÆ?°u¸£¾ï;?ëÓæ·ã`?°u¸£¾ï;?´lTû¥•`?›È•!é‹?íru`TS"?›È•!é‹?p£ï؛Z5?¨±É*ÈÃ?ïÞ¸ ‡"ã?¨±É*ÈÃ?xô•kÊý?†¯šN</?ïÎÕ?É*?†¯šN</?ˆã+âEª»?yHÔ¿éD?ïœsP"§Å?yHÔ¿éD?YÏòöÉ÷¹?LT¤;Å?ïóm=¬?LT¤;ÅPSR3FGL J1900.8+0337@BœæB¿˜1¿Û£Òm¾À7°]«¬Á•À9ñïÞIÍ?þ9ì$ÖÏ@›,ªØÜ%@͵^q$…¿ÓfÙJVê¿êt–Ë'–ô¿èèæç]п/âØõUNASNone@Ðª0U2aLogParabola	?A$Ca^w?JÑB¨ë«?ïû¶úÓpU?JÑB¨ë«? %:Oß?º5´Ø9g€?îÿݯ·×â?º5´Ø9g€?É#å ¶Ìä?°%5)陝?é·—ÒLÇ?°%5)陝?²ÀØ]Ùã?"bi0åÿ?í§ÿDæ†T?"bi0åÿ?fZì"ô4Œ?r×³î?ïé¥[¬?r×³î?ƒØX·ø7ˆ?¥xÌæM'?ﰞ(^2?¥xÌæM'?ˉÁÆp?¶þl'åA?é8<]Žd?¶þl'åA?…eÙT˜Ô:?q—ZC%@B?ïªhš"a_?q—ZC%@BPSRøø€øMIXED@#Ð8½
ã4FGL J2027.0+2811@Q5Kaþ!ÙÀ‡oó­â&À9¬ŠS«x¿À<©"àß@Ans{!ß@z*ž9;‹?Á *†<ð?ë7ZU¶ì@!ýAØèd@YøŠ•Æ?ïû/²?¶Âa C?¿Ü7e\{+¿íô×x!yÍ¿ï÷M@ÝÁ¿ïÎ߁Z]šUNASNone3FGL J2026.8+2813?«aÆrÚVè?¹#ë<…‰›?îI㘍¢b?¹#ë<…‰›?¯‡¡_æ¹k?²Al¢cÄ?î…éʚª?²Al¢cÄ?È;Ÿpü ?®¸`h§\›?éñ#ÀØ?®¸`h§\›?¡É6Ø=Ë?‰–/ôè´?îãl'`¦o?‰–/ôè´?|Œ­å0?À\ÉØYP‡?ïš²•¶?À\ÉØYP‡?ˆç²9FÇ?–ªŽ»B?ïœa7R|¥?–ªŽ»B?¼Y±)á®?­œFgÛk?ì|ôÉÚÃÊ?­œFgÛk?Mìã³.fv?>ûb‹8S?ïø"Ç-.??>ûb‹8SPSR3FGL J2026.8+2813@Q5éÍ³}ÀK5°»õÀ9˜d
ƒ À;:†œfÓt?õà—Ê·sÊ@ᓿºëy?ùj§ŽN⼿â2kü¿Òs=idj¿ï†)ñk¿ïýGwtUNASNone@Š}ÔA5TvLogParabola?·[ea›µÚ?¾D°H²¡R?í"S•…?¾D°H²¡R?»\´Bߚý?žWá¾?ì"iw¤ ?žWá¾?܂ÿ€ËŽ×?´Ó9ôj?ᾀ?š8•?´Ó9ôj?Íõù- C¤?«Q`3¶)·?肁´—ï?«Q`3¶)·?–…&2(M$?­ú=|bQ?ïKÖÎ`ÿ'?­ú=|bQ?"/«ý?©ÖÜ
Ñkø?ï_÷>^‡?©ÖÜ
Ñkø?é¤Óç¸?«êç².Ðs?ë–üË?«êç².Ðs?™38ÅÜ?€ê‡=Ž?ï{6gE3'?€ê‡=ŽPSRøø€øPSR@Ã=ž=¤4FGL J2038.4+4212@Ta¼©iv?á^wïû¥þÀ7çÇҒ¬À:6ÃákÀ@–¾Xéò@9Ó{<·@?·ÿvä܎?Ø+L'Œ@ ¤zž+Ð@‰ý¡O?èJ*Æ}'s¿Þ/–Æ€'q¿èHüލi‹¿éº\‡ÀSB¿îSfQÒ[¿É½‹¦¼Â¿UNASNone3FGL J2038.4+4212?Á$<¨Û^"?ÊÄ1'õ·?ë¶ðÕÉ([?ÊÄ1'õ·?±7ם5Z€?±¢vÙmr‰?íÙYT°?±¢vÙmr‰?ÑßÑ%;?¶{}EÛ>p?çqymc?¶{}EÛ>p?'Tæ8·4?~R×腢?ïm_0‰'?~R×腢?ÒO-ü"áè?אÛ.dl?æØiî?אÛ.dl?…dny?Í`ãž	;?﫟º‰Âü?Í`ãž	;?ųyÌl!3?´KªÍuÝ?ê"!Œä÷³?´KªÍuÝ?Mÿ}.Þ?…ã·Çƒ?ïÿ%™?…ã·ÇƒPSR3FGL J2038.4+4212@TaÄØì–?á]iR‹¾À7ö;¤ñ¼pÀ:ûwÛð?ÿSÊ7F=Q@'<§P;'?ýC7àlõ¿¶ÕA™(¿åæà/'N¿ç°—já¿é8‹ÛÀÛUNASNone@™Ì™‡+LogParabola?l3ûÕ*î±?{üB7ˆY?ïãÌèܒ?{üB7ˆY?«,KN½:N?¾¨(VúýQ?îM;Jêñ?¾¨(VúýQ?ÐN??³µ`WU<Î?çˆ23Xòà?³µ`WU<Î?ÀZ?•Ûã°?ÔÊF?ëép‰?ÔÊF?`gÖ5#ËÔ?cö$?ïï˜)éÄ?cö$?(ŸÐM1w?¨œâZoæ?ï~»¦ÑÄ?¨œâZoæ?¿8ïÏu
?µÎÁix[à?ì˜â^?µÎÁix[à?•Ä»Î{7T?Hgœú%»?ïQÚ!bêö?Hgœú%»PSRøø€øMIXED@iÛŒÙ4FGL J2112.5-3043@-ÎÈ`VíÀE8Ɔ"ÄÀ8¹}'âïÀ;ûK¯Ri@æDÖ ³?ù?<;±'?«é³@pž?݁b ß9@1== ò¾Ï@'wVM¿|¿Ý¸çì
?¿ç¨eÜÔ¿ÄTÌ '¿àã|aO{=¿í/à˜[¬¿ïÿý±q&´UNASNone3FGL J2112.5-3044?hã)rüŠ?vo*mÜcX?ïçÖiG†?vo*mÜcX?¾ê¥®Xv?ÂÍ<w.Ï?ì"«J4ñ=?ÂÍ<w.Ï?¨ÞÆÁ½F"?œ®g™Ý°L?îr"ä+—?œ®g™Ý°L?@ú
¼$??»5‡ÀjÔ?ïûÁ}Þ??»5‡ÀjÔ?>,]‹§?¹&{Ï£#®?ïƒN}ça?¹&{Ï£#®?™Ê¡³ËG\?¥F…V/{?ï1ªòSçU?¥F…V/{?±bûÈcû?¦M:¼±?íÓ ]¸1?¦M:¼±>½Wjú@Ç6>ÈųQ»?ïÿüUE7>ÈųQ»PSR3FGL J2112.5-3044@-Ì`RP/ÀE9nÀY!À8¯¨tþ¯žÀ;N%@+i:@ABŽ@•ä¯—‡Ç?ñĐ£PҀ¿ºTqu§æ¨¿ÐSF"ã!M¿áG¡>Ô|¿ïÿù_|è3UNASNone@'¶¡ÊÀƒLogParabola? áz-Ð?±¼õ1æo?îÿ¡ïºž³?±¼õ1æo?DZiÇl¬?Ò}¿ZÒ?ꥎ;äÕ?Ò}¿ZÒ?³2Ïùç2?¤2XÐx>Z?홦¥F:?¤2XÐx>Z?¯‰AÞ·e?"²èq?îkïÙ:?"²èq?¯§àªj?ÁÞâT"¢Î?îU',Yi?ÁÞâT"¢Î?»…Ul'?ÎÉÄã'
?ìU^'m½?ÎÉÄã'
?¥E9ú?¡
"B×·?î¦/û¬op?¡
"B×·?†.2èGŸ?u¥ùªÍ‡Ö?ï§G7¦²?u¥ùªÍ‡ÖPSR@sâfffffÀ>µÔò¡56, 60, 60,60,60,60g@Vó…;˜PSR@gæÑþx

==> SOM_VIZIER/3FGL_prob_catalog_2classes <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  431 / width of table in bytes                        NAXIS2  =                 3034 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   52 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\3FGL_prob_catalog_2...'TTYPE1  = 'Source_Name_3FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON    '           / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Signif_Curve)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'ln(Variability_Index)' / label for column 7                          TFORM7  = 'D       '           / format for column 7                            TTYPE8  = '500MeV_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'HR12    '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'HR23    '           / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'HR34    '           / label for column 11                            TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR45    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'Category_3FGL'      / label for column 13                            TFORM13 = '5A      '           / format for column 13                           TTYPE14 = 'CLASS_3FGL'         / label for column 14                            TFORM14 = '5A      '           / format for column 14                           TTYPE15 = 'Pivot_Energy'       / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'Spectrum_Type'      / label for column 16                            TFORM16 = '16A     '           / format for column 16                           TTYPE17 = 'ASSOC1  '           / label for column 17                            TFORM17 = '26A     '           / format for column 17                           TTYPE18 = 'Flags_3FGL'         / label for column 18                            TFORM18 = 'I       '           / format for column 18                           TTYPE19 = 'AGN_BDT '           / label for column 19                            TFORM19 = 'D       '           / format for column 19                           TTYPE20 = 'AGN_BDT_STD'        / label for column 20                            TFORM20 = 'D       '           / format for column 20                           TTYPE21 = 'PSR_BDT '           / label for column 21                            TFORM21 = 'D       '           / format for column 21                           TTYPE22 = 'PSR_BDT_STD'        / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_NN  '           / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'AGN_NN_STD'         / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_NN  '           / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'PSR_NN_STD'         / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'AGN_RF  '           / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'AGN_RF_STD'         / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'PSR_RF  '           / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'PSR_RF_STD'         / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'AGN_LR  '           / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'AGN_LR_STD'         / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'PSR_LR  '           / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'PSR_LR_STD'         / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_BDT_O'          / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'AGN_BDT_STD_O'      / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_BDT_O'          / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'PSR_BDT_STD_O'      / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'AGN_NN_O'           / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'AGN_NN_STD_O'       / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'PSR_NN_O'           / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'PSR_NN_STD_O'       / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'AGN_RF_O'           / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'AGN_RF_STD_O'       / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'PSR_RF_O'           / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'PSR_RF_STD_O'       / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'AGN_LR_O'           / label for column 47                            TFORM47 = 'D       '           / format for column 47                           TTYPE48 = 'AGN_LR_STD_O'       / label for column 48                            TFORM48 = 'D       '           / format for column 48                           TTYPE49 = 'PSR_LR_O'           / label for column 49                            TFORM49 = 'D       '           / format for column 49                           TTYPE50 = 'PSR_LR_STD_O'       / label for column 50                            TFORM50 = 'D       '           / format for column 50                           TTYPE51 = 'Missing_Values_Flag' / label for column 51                           TFORM51 = 'I       '           / format for column 51                           TTYPE52 = 'Category_Prob'      / label for column 52                            TFORM52 = '5A      '           / format for column 52                           DATE-HDU= '2022-01-29T22:21:14' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             3FGL J0001.0+6314@]RÂÀð ?íŸWÿÎàVÀ9ZzŸÙOÀ:ÿ!Z³¿õÆkvñxÿ@Å "	¸@ܾßú&!¿ç0WìPӿ쳊Ügu¿ÜƒûÂكê¿îæý/k'–OTHERspp@}'€PowerLaw?תּÒ"ïf?"Iµ®·ÿ?"Kˆr2€?"Iµ®·ÿ?ïÀà^5P«?ì¯˜>?Ðë~²?ì¯˜>?íJR9o?¤1²Lo?·¯Ž¸?¤1²Lo?ïÿI: S·?'Ƒ?ئI½–Ð?'Ƒ?ïG3Œ/´à?Ÿáˆáé?—Ž€èœ?Ÿáˆáé?î¡­LÔ?µ},L¸`?¥î52~çÃ?µ},L¸`?ë¨} "p~?­×;"oZ?Á^v>?­×;"oZ?ïôþ"ôæ`?S¸K+é?V¹°~Ð"?S¸K+éAGN3FGL J0001.2-0748@VAk¿×ÀPÔÀ€"ÐÀ9"ñóÍÃÀ;¯Þ>Xˆ?ä‹|¸&;@Avû	 @1݀#Pè¿ÔÇZö#eé¿ã+ùÖζå¿Û5šÜdÅR¿í›Q÷æÎAGNbll@"¿Wö+jèPowerLawPMN J0001-0746?ïTîÌ»ý?•#CÉOâ
?•b<H NV?•#CÉOâ
?ï\O©Áã?¯Ãqˆ6Ì?"v*ÇÒ?¯Ãqˆ6Ì?ëbÀ¬X?©\U[:»?ÂwǬýN ?©\U[:»?î¦'˜?Œåœ«àA?¯Ež×²^+?Œåœ«àA?ëì'q/å?»±r¾àÀ?ÀM»â;@j?»±r¾àÀ?ë–:~xxY?ƨ€«ü?Á§›?ƨ€«ü?éÄ=úŒxŸ?°YA´²"?ÈïÎ…?°YA´²"?æ•Äe¨®é?´éSoé«?ÒÔw4®¢.?´éSoé«AGN3FGL J0001.4+2120@Zê–_RuïÀD	@¢CÀ9‹!P²ŸûÀ;ÎÑPÀô?÷ÁF#zÙe@{J¨š¾@d´¢´uh¿ã©OºÛç%¿êJJAuHà¿ïÿ:ÕÇ?º{	¥_rAGNfsrq@sjèÍJ¡LogParabolaTXS 2358+209?ïÿS±œ´p?ÿE©?‰Ä`ë5
?ÿE©?ïÁۖ'ý?Ž±%Õóô?4Éø?Ž±%Õóô?ï1	ßfé?'ºÁÑSì¨?™Þݛ|Ü?'ºÁÑSì¨?ïÑv	ˆ?jŒŠçøëÅ?wDûZõ\?jŒŠçøëÅ?ïÿ=µ·u?&ï§'?If'z''?&ï§'?"Ã?±èñTBVÐ?¤f·µ‡ˆ?±èñTBVÐ?ï
'·³?—Ê
Þ8,?Ÿ>½èÉќ?—Ê
Þ8,?M¶Ë?©Æ˜¹ÌtJ?¦Tf)lÅW?©Æ˜¹ÌtJAGN3FGL J0002.2-4152@tá !¸ÀR	"`¸À:†¾š§·À<˜¡L'¿ùº­ Œ§ï@ \2°@¶ÆCò¿éÖ%8ý*@¿çž>éí‡?±Dņ YÖ¿â"yq…ÿ3AGNbcu@ž*~ùÛ#PowerLaw1RXS J000135.5-415519?ïÿ‰Ð£Æï?‰8v¦—o?
‹ÔC$èE?‰8v¦—o?ïÕP9±Û
?Ðn¥¡¦?uWã,'Ù´?Ðn¥¡¦?ïé§]žãþ?gL·ÆÜÅ?fX¢Z<ÊQ?gL·ÆÜÅ?ïÿú<­Á€>ÀcœêªOœ>Ç®ôüW>ÀcœêªOœ?ïÿµ(ìÍ?€E159é?½.ñ{?€E159é?ïj5û†ëä?«ªx 8‰Ó?'¹@ÚQq?«ªx 8‰Ó?ïàìî¥{?y#4_ȅ?oÆ5Z?y#4_ȅ?ïÿÛì©À>óSsh3û>òuƒ§ÏCH>óSsh3ûAGN3FGL J0003.2-5246@sïž?»×²ÀOiÿ¼ä!À:‡¯»DMÀ;èK	éÎ¿¸otpl@€Ä©Ü¡?þRÅ؈B¿ïýñ$yœ?ﶰÅýr)¿ÙjÓ³'	¿Ý¾_îõcAGNbcu@¬¸t!-wPowerLawRBS 0006?ïþڔdzï?ûê!tËY?"V³ÎÉá?ûê!tËY?ïϛ«æ?ŽBja1n?x2*4]?ŽBja1n?ïÎ6,?©?~@€uF®.?xäéØ°«?~@€uF®.?ïóÛKœ?F?&<h%ý?XIi0X.?F?&<h%ý?ïþG>êÖ?.HTpíó?+ŒÜÓ?.HTpíó?ï)ÛRT?¯ÕÕßðëæ?šÄtÇv?¯ÕÕßðëæ?ïÊ!"úÑ?'P¹½¥¹?zï?Iá/c?'P¹½¥¹?ï®3{qTE?wC£t`
€?"s!ã\Ë?wC£t`
€AGN3FGL J0003.8-1151@U¤ YÀQÅcÿï9À:¬"V;uøÀ;ù è­Óã?âŸ8ÅCk@
¢'<@0+ÿ>l?éyÑyý‰¿ØóK^¿åD:Ï<q¿Ü¼ûßðýAGNbcu@¢Á½¥PowerLawPMN J0004-1148?ïþ°÷P¦?.¬¿eÈUŽ?/ôî4Ó7W?.¬¿eÈUŽ?ïÃqç£è¨?äˆybvÖ?~GNWÿÙ?äˆybvÖ?t$PS?'¦'bµ?ˆVãª[I?'¦'bµ?ノ#L-?dë#{
‡u?€~ÇS·?dë#{
‡u?ïù.ˆ©‡?JÖÑÁ"I?KóFÒž¢?JÖÑÁ"I?îÈí¹EJQ?µÎªàxW(?£q$jÏsõ?µÎªàxW(?îÍÇ&Ö¿¦?œÅtîÞRX?£#•'ºœ?œÅtîÞRX?îxÉ5Wj?šDÚ V‹?¨i:íl?šDÚ V‹AGN3FGL J0004.7-4740@t=Ÿ¶MÀPá1ÔÌvÀ9iÎ,H]gÀ;؂—õT«?ãqP7®u§@è<Vžó@:f¿§ C¿áMwé+ä¿æXÜZ½³¿äXzLnºë¿ïÿð¸å9UAGNfsrq@†"Ì?>qPowerLawPKS 0002-478?ïتh@S?$'·Op?sóª¾!fÂ?$'·Op?ïÉkº»í?ì}1Ó
Ž?{Juªá}?ì}1Ó
Ž?î
yÃ†?¢aê6?,?¯VøgãǙ?¢aê6?,?  I?pn?Å[?Š™×Æ¿±J?pn?Å[?ïóKšÄM3?l+§ä6&'?YhÊâ™j-?l+§ä6&'?îÓõ«ÆË_?²ZÃ6…?¢À¥C"J?²ZÃ6…?íöZ³»êã?¢©Ä¤©$ù?°M*a²µe?¢©Ä¤©$ù?íZ,—ôº
?¢ë­h§Šþ?µ.›>¢a›?¢ë­h§ŠþAGN3FGL J0006.4+3825@\U=žÇÀ7‹@;À9Jn¿Ñ;ÇÀ;™2"Ѽ?êXyç¼V@&í @ïဎæ¿çGkÚ¢+¿æÝH
1ÿìNC–œ}é¿äz"&V½AGNfsrq@lß&k¥PowerLawS4 0003+38?ïÿõ$¸O?0@•)¿,¤?á^ûÁU»?0@•)¿,¤?ï¢$=T§Ö?'´ÒJÔN?‡vð£öÒ ?'´ÒJÔN?ï´Jq	Ð?ƒ¸T7O‰?'ùíV¯?ƒ¸T7O‰?ï+j×ö]?yú&O?šò£Ifh?yú&O?ïûb_×½'?Dí¦xsùJ?Bv€k·ÚÎ?Dí¦xsùJ?í§z›7æ?³À0"Wz?²Ç+"4S?³À0"Wz?ïp}"yÌ?ŽÏDµâ[?'ð[¼!*ˆ?ŽÏDµâ[?éºc°î?²ÉS[ís?Ë­êq<G?²ÉS[ísAGN3FGL J0007.0+7302@]ê_á'p@$ëÎ ‰ãCÀ5"á÷|þÀ:H!ß&¡@ö%/Íù@¨Œá¥Kÿ?øè!¼é)û¿É_:@KRA¿ÙyB+s¡7¿à掝¿êwë1olRPSRPSR@Œ­VPLSuperExpCutoffLAT PSR J0007+7303?rµ4¡½•z?šú"òÁɧ?ïڕ–ï_
?šú"òÁɧ?©áŸo ?ÀÌ#yײY?înñîMÆ?ÀÌ#yײY?½ž)œí8?­+´Ö	W/?ìL:ÌbLY?­+´Ö	W/?-åp}åg?"¸oQf÷ƒ?ïþ!©B?"¸oQf÷ƒ?~‡ˆ-48e?©$©]«­?ïÂðﰖO?©$©]«­?"CnfPq&?¯€®º]Ìs?ï]䌱ÿ—?¯€®º]Ìs?˜¨‹ßM¬&?˜¶VBö­m?ï:»¡<Œ_?˜¶VBö­m?_U	íû?¶žÛ¦º¼?ïÿ¦ƒ·Úø?¶žÛ¦º¼PSR3FGL J0008.0+4713@\ÕH˒:À.WÊÆbÀ8‹e²€gÀ;<µgUy¯?íñvi,®@Ó=…Ï@+?ëÓM¿ÀvþF
ø³¿àœ €Ò[¿Ú̀èYˆ¿äC9qzAGNbll@NÒñ©ûçPowerLawMG4 J000800+4712?ï\ÿÄ_¯­?™Hú`Qü?"`nâ o?™Hú`Qü?æX¨gŠK?ʸÍHjy?ÓN¯0ëÁk?ʸÍHjy?ïÀ܇2—?'ï ýµ#Ã?žçäf'§ ?'ï ýµ#Ã?çT[&?¨Yi4ÄOG?ÑWIɳÎà?¨Yi4ÄOG?ì³[i³"?¸³A²é&?ºe$²fïù?¸³A²é&?Ð7½·í'ò?˪"I?çä!$	l?˪"I?í´ "±9?ªGS4\2n?·j^ú삻?ªGS4\2n?Ð1Ýj Q§?¯ž~)ØiÚ?ççJï×-?¯ž~)ØiÚMIXED3FGL J0008.6-2340@I#ڿԖÆÀSð*ùš‹À:c)ÒaaDÀ;¯S;ç6Û¿Äû¢£-—@ÜAƆb?ù•<@5? °ò?'Õ?ïüz¨£Þӿ窜>öœ?Ú£¤6¢ö²AGNbll@½ã×
=qPowerLawRBS 0016?ïüž¬Üu?Gªx¦àmK?;
™8í¹;?Gªx¦àmK?ïÖy5ïK?†ÝÏ®o?tÃeŽ…Úl?†ÝÏ®o?ï\l®î¯:?‰â²É2¼Õ?"rj*ÁÄ?‰â²É2¼Õ?ïÿH¶çÏ?öt²NBf?é@"VÈÑ?öt²NBf?ïñauՈø?ec'A¥®?]=۞¿¦?ec'A¥®?ï‹2%3?žZ*ëQw`?3X¥''8?žZ*ëQw`?îBbKWIñ?¡[p^MB?«ÙÛJ‹`é?¡[p^MB?ïø¹*óZ?Q§9Úµ^?MìW?Q§9Úµ^AGN3FGL J0009.1+0630@ZMa²¢ÀKlR@>´qÀ9Íêï̓À;µþÓ°Ý¿ïæJ˪@w"²î'@oV@S'3¿àmíóQá¿ã-˜û¿áW¹aÏÿàŒ*h¼àyAGNbll@˜3á–R½<PowerLawCRATES J000903.95+062821.5?ïÿ{Êg?âÚCöÌ?†Æÿ;ˆ?âÚCöÌ?ï˾E?Bõò*Â[?z ÿù¥Àë?Bõò*Â[?ï⒬j©?v¾~ÿ?mmSÍ×î¥?v¾~ÿ?ïÿ«¼†Ùy>û6L‰Z?àÌ p>û6L‰Z?ïÿ<Õ¸«?x%óîÏ?eO˜ÈßW?x%óîÏ?ï(í Ì ¤?³áô‰ü®í?šâ[ÝÔå~?³áô‰ü®í?ïȳõ²Á€?¯'¼Ê
?{¦Wó?¯'¼Ê
?ïü(àIz?6l¶,ߖ¨?>¸ü"?6l¶,ߖ¨AGN3FGL J0009.3+5030@]s`Iì³À'›I ÛAÛÀ8ҍÖí¸À:ú€ÌC:?èNêj±="@e鋁 ?þÛ°àˆŽ¿á"¢x1¿Þ&úÓùÅ\¿Ù͹"¤³¿âQ®Ñí§AGNbll@™ãÔã¼Ó[PowerLawNVSS J000922+503028?ïÿ"Ól¼?
p/Zó•L?Ë3ô+ív?
p/Zó•L?ï¯|üB?m™-'X?" ÁÞ\O?m™-'X?ïãýÊX?qŸ)CwÑV?lñÅÚЩ?qŸ)CwÑV?ﳃbÿc?b›-0ý[Z?ƒ'=Ö­%?b›-0ý[Z?ïþmoU^'?%šûڌ^?))
TSÌÎ?%šûڌ^?î>w©§%@?³ÆLö'äö?¬…e¬?³ÆLö'äö?ïÒ£575?&Í=šÉ$?v®e‹Ñ&?&Í=šÉ$?îǁ-‰r|?ŒÕ»X½"¹?£‡í%±
<?ŒÕ»X½"¹AGN3FGL J0009.6-3211?ôÒÆ>¾ÀS愠
Q!À:iÁµA•ÍÀ<YQªí?›¹ÉŽ©H@™ÎØÿ@zSŸd^Ͽ〠ƒ¿ãô](5dw¿æ¶"Ò
¿äbzª¨hAGNbcu@·B&€IPowerLawIC 1531?ïúàô÷ä?Z¦I/'?Gà|̧È?Z¦I/'?ïÎÅ6ÄZ?•æ+ÿžlx?xe:;?•æ+ÿžlx?ï@/£?–¤	;lø?œ°ôä$?–¤	;lø?ïÞYTì'?XdN"#Â4?p÷S3ÝÀÏ?XdN"#Â4?ï🰒?k`òm{õ?^ÀžQuy»?k`òm{õ?ï7aAI²?§Þ)D¹4?™×Î2¨t?§Þ)D¹4?íÙ{¡¶ôs?¦gå¥2jf?±4"ñluf?¦gå¥2jf?îj¼ßh¥?–­Ö#Èf?©T2‰Ù°?–­Ö#ÈfAGN3FGL J0012.4+7040@]ëþ?5Ÿõ@ Ì <ÁÀ9Ê ™ÙZÀ;KÀæå|Ç¿ù¦®ÕëÚ@‹`Þj.@Þ¸@xÁ¿ã
Q2L®¿ëÓP¹?
¿â1Àª³%¿ÜGÐç—1AGNbcu@«]—ö+kPowerLawTXS 0008+704?ïÿŠÊÒTT?ê»r«¤¬?
MTߚ]?ê»r«¤¬?ïЯ"q€e?†¶5/X?w¨5âÁ"?†¶5/X?ïå ¯H¾œ?\êTðæ¾+?j_PÑ^kî?\êTðæ¾+?ïÿ󎾰f>ІHs¿íx>Øây½8">ІHs¿íx?ïÿv¸÷‹p?%<H9?(é~ݗ?%<H9?ï	Ht/t?±l{'î;?žÝÖñzz?±l{'î;?ï·-'DV`?Ä)–KŽM?'4¶9é'ó?Ä)–KŽM?ïÿDp?§ÞRí'?Øùjœ?§ÞRí'AGN3FGL J0013.2-3954@tÅ.@…+NÀR½"@(äüÀ9¯ó¢#«×À;ÛÞ|!¹Ž¿þ)
Ðx(@¿(Ÿ[z@±»€Hj¿â4¨©,	¿ä+P)§Þ¿â¹).<¿Ös³Èç1tAGNbll@'ÎàÞ҉PowerLawPKS 0010-401?ïþJ_cž?3QwÑ??+Zöžƒ°?3QwÑ??ïÞºŸg}¬?ƒBãK‰¬??p¢°CR-Ö?ƒBãK‰¬??ïÜ"ü?u)›¦Ú_à?qöv
;¡Ð?u)›¦Ú_à?ïÿù¦äI°>ÆHç}XØý>Éc¡žŠ0T>ÆHç}XØý?ïþRt¨/?(°-oÁF´?'*Ù¥.ŸA?(°-oÁF´?ïÊ4cQ?¢ÔºOCJˆ?rÙa;Ì?¢ÔºOCJˆ?ï¯Âzcs?‡B4ì{?";OhöG?‡B4ì{?ïÿsåÍF<?}ŠŽ;;?ƒIA'¾?}ŠŽ;;AGN3FGL J0013.9-1853@R¨øäÀS…€,á
À:¢ÐqœûNÀ;þ¦Ë±CÚ?ß!0wþ$š@Äû—»s?þö`¾ø?ïøÀá\%ñ?Õæ/–½é|¿ÚëlÌVo¿êǦ—}"AGNbll@¦8ÍÒñ©üPowerLawRBS 0030?ïÞ-ê–Y?°ã2³Q=Å?Ÿ¤:=…Êï?°ã2³Q=Å?ïZ³¼@Ê?£9àÉÊ]?"¼é…JÏ?£9àÉÊ]?ì²yˆ¾;?§³JM_?ºoü3º&?§³JM_?îHfÞRӄ?í.Ôßô?«y'ùÄ?í.Ôßô?ï@¿µ? a?†¹Ô3?ž—è<)Z? a?†¹Ô3?íª–Zä—?ÂH˺—ÚÁ?·j«LLôJ?ÂH˺—ÚÁ?ìA*Îp÷ö?¨ÈpKáb®?½ö©Œx@P?¨ÈpKáb®?éõÑl³v?´q
±Ä9ª?˘(ºM2'?´q
±Ä9ªAGN3FGL J0014.0-5025@s×7À*ýÛÀPh"  0øÀ:™û3èdÙÀ<0{ÈÎ;?×Ɵw»3®@±Ëžðñ?þÈ3€5'¿ç§vóÁ.¿ÑÔ'54P{¿ä/çP~$¿ÜºhÆïƒAGNbll@¦Äÿ—$tPowerLawRBS 0032?ïýYyëÆ?3At"¯ÐR?545è%<à?3At"¯ÐR?ïÄïiŽ˜?'ÄÈo»'Ë?}ˆ{ÚVü#?'ÄÈo»'Ë?ïÅHð~?~ŒÍvG‡b?}u[z8Ñ?~ŒÍvG‡b?ï×ýH{Õõ?Yύ»LÄ??t[¢xn?Yύ»LÄ??ïú:ö˜oš?CeªüQÃ?G$º‡¬?CeªüQÃ?îê-,«Q?³@¹"u¹ù?¡]-8ºŠ?³@¹"u¹ù?ï³ÞQ¸)?ƒÜI	º»?ƒk—$_¶?ƒÜI	º»?îkrPÉ?—òÕ¹Ê*u?©HÛs‹?—òÕ¹Ê*uAGN3FGL J0014.6+6119@]¡ñ'l¿óÑ=ŸÈ²·À9"=ëóفÀ;QÙ($â8?ìqÌ[ã¬@k¾vçÂ?þ3#Þ¬s;?î'NË®Ùa¿µ™^'Ÿ"¿ÑÃñ)è ¿ÝWGph.#AGNbcu@´Cÿ;dZPowerLaw4C +60.01?ïôç5XÒT?SYqºp<s?V1•ÏŒ§?SYqºp<s?ï90…%e¸?£+%ű?˜ÙïV+ß?£+%ű?諭ZÕ?~ŠÜ«?…yPƒ8Î?~ŠÜ«?ï+î²Ð¢?{0°‰6«Q?šœ"ƳÁ?{0°‰6«Q?ïÚm£Þc?n}_~L*‹?rÉ.Àº¦?n}_~L*‹?ì5iæ†?Ãè‹(Vz$?¾WÔ°ÏsÏ?Ãè‹(Vz$?ï$ñdíѐ?"ñÞSÓ?›aÓcý›ñ?"ñÞSÓ?í°Ð t‡Å?œÍ@ñ|Ë?²yzý7¨Ø?œÍ@ñ|ËAGN3FGL J0014.7+5802@]"Ñ_ÄÖÀîQ`Dä6À:.[)òBÀ;'Y5%{»¿ÙN´þúÇ\@
i•ûg¿?þšåŸ¶´?퐗Ã^B?ꎽ¢ãD]¿á>Ö¿áA"HŸkAGNbll@¶-b¶®PowerLaw1RXS J001442.2+580201?ïþMƒž£?(°M‹´3»?+'ÊރÙ?(°M‹´3»?ï¶eYöì[?ŒfoÞ¼?'f©'(?ŒfoÞ¼?ïЦ ­Ï?u¹ÈJËm	?w¬ÿ8˜?u¹ÈJËm	?ïóWdüë?Gž{§%~V?YÅP¯Uz©?Gž{§%~V?ïú‰¿9™Ý?BÓ%º?EÙƒ™C?BÓ%º?înнÈ"?¶ÎóÒ®‡?©ô&ízx?¶ÎóÒ®‡?«rt?"bgaZß?‡ž•ðú?"bgaZß?ï–%Ùè?…>ÉÆ0q$?Šyö®K$?…>ÉÆ0q$AGN3FGL J0015.7+5552@]z,¾¤ëÝÀ˜>àŸ°À:])¦ÂwÀ;§UCÿ3?¥¼RX‹‰@

a'Ñ×@êÀ/¿ã•ÖÞ¾¿æ®ëFÏ6"¿âªƒ&:§F¿âÓ´`ÖjÁAGNbcu@§uþ\'ÑNPowerLawGB6 J0015+5551?ïÿdœóÒ?dŠ¯ß¦?"nÖqd]?dŠ¯ß¦?ï¤b³(‹å?•ÄW½"<?†çSG"?•ÄW½"<?ïæX7ŠÁ÷?_P'
eæ?i§È"z™@?_P'
eæ?ï×à,-¸þ?[I²æƗÚ?téûx±?[I²æƗÚ?ïü»:å?q?8l(íØU?:&)âL`N?8l(íØU?íÚs€¢Ÿ?¸Æɪ8?±ã,bC	?¸Æɪ8?ïÇw…"÷?~ášb?|}D-gPv?~ášb?î1Uãad?ŸuÌMÎ?¯üê¡ÉéÃ?ŸuÌMÎAGN3FGL J0016.3-0013@ZáuÑ=ÀNç…`&±EÀ9;ŸDÔEgÀ;¶QºÝ·?ó¢xËmÒ@±vÚý½@ñ]À¥w¿ã¼²Læ/¿éq`œfÂF¿í¨Âñ¤¿ÖÆQ÷!<ÄAGNfsrq@|{žPowerLawS3 0013-00?ïÿz'Û?{èFßeö?¯Å#íâ?{èFßeö?ïÍ*;‡?‰/}rÑÁš?yrêÖ¨'?‰/}rÑÁš?ßÌêæ?‰¼v4D?SH	Uª‡?‰¼v4D?ïËÁAÃ?c¸ºîW|?zrö"Îx?c¸ºîW|?ïÿBxÔØ? b,›R1²?°íº§o? b,›R1²?îþ™À}UŽ?°û¾"¡%æ? cùŽ%?°û¾"¡%æ?ïy½64x
?@¸ú)s¹?ÈY@P6«?@¸ú)s¹?îÜ´,S+\?›Öâ0~{p?¢4½=`ÿ6?›Öâ0~{pAGN3FGL J0017.2-0643@XêÉ`0Â@ÀQSÙÔóÀ:*V]çÀ;Ï% £y¿«NÐÅMŽ@øœJNì@íø@˜÷]? R
Œçã¿ÅrdgnàD¿æhuµ8Ü¿è¯4Ã×ßAGNbcu@ÇäxGPowerLawPMN J0017-0650?ïì;Cß?idçÙ>/q?cøÄûYÁ?idçÙ>/q?ïÍ)î³Hå?‰"hÀ#j??yk¸9…›?‰"hÀ#j??ï]ï®`P?ˆ_Ý1à?"BŠ3õü?ˆ_Ý1à?ï®q½©ç?l\9g:P?"yc€fs?l\9g:P?ﹰܒxÏ?†ÙfÓS?"ÈãøÒ(?†ÙfÓS?î˜O¹¯A?¶Ciþ¼Ä?¦ûÑVî?¶Ciþ¼Ä?íþόM^`?¢Ô쉉3Î?°	ƒ›Ý??¢Ô쉉3Î?ìP&àNÏ?¨Ç'ø«ýé?½~Ìý‰Œ?¨Ç'ø«ýéAGN3FGL J0017.6-0512@YPŠŸb0ÀP©&¿òÉ·À9)´xB0ýÀ;cî4üa?ãÂÇàÔÁŽ@Àù™´qŒ@áÀ#ñø¿äÜEZ…»¿æéú`"üb¿êvºÏý·¿àÏÀÙ5AGNFSRQ@Šé|ÚQPowerLawPMN J0017-0512?ïÿ­ô‰C$?;Î~¬6Å?'íß
âò?;Î~¬6Å?ïÌÎ듔û?"áyàs£?y˜Š@"VF?"áyàs£?ïÆaem™?€FÕÞ`¡j?|ÏM(|sã?€FÕÞ`¡j?ïýߦ*?)•¡ršÌ?1ρjîk?)•¡ršÌ?ïÿ{£F8?yI5'ö?œowܙD?yI5'ö?ïBiÈ4Y?©"r-(‰	?—²Ü@<æ?©"r-(‰	?ïƒ?ÒÒn?‰PìºOˆ?0oü€?‰PìºOˆ?ïøoW`å?D"¦ë ?NC›㒧?D"¦ë AGN3FGL J0018.4+2947@\›¨d©ÎÀ@Dߥ¥À:´Ÿê$ÌÀ;ú"#—µÀqÌMËåÇ@r÷na?ýÕ
ÁÉR?ìQ+êr,Ì¿êàƒKà^¿ÅAí§"¼¿Æ(·±TÒAGNbll@²pcŠ	PowerLawRBS 0042?ïÿÂ)I"7>øƤ4=¶>þëoÊí>øƤ4=¶?ïÝ`
¹(?|ÈrqúÖ?qOúؐ‡È?|ÈrqúÖ?ïê|1m¥?cL2»T-?eƒÎšš?cL2»T-?ïÿÿ䞝>gڌp—Š>kŒUnlmÙ>gڌp—Š?ïÿâÖ=Ô>øÕmMRL>í€ÁJW±>øÕmMRL?ï3T( Z"?³Õ [fÄ_?™•{Óåˆ?³Õ [fÄ_?ïêtþQ?hæ¡Þ W?ep‹ßÃÞµ?hæ¡Þ W?ïÿþæ$Œ§>±"¿«¸$Ò>¡¡2êï	>±"¿«¸$ÒAGN3FGL J0018.9-8152@sH _ñØÀA"á@!X?À9¦8‰´IHÀ;©‹K"=B¿ò½¡ÜF@ÍnkB™@š€ ¤OÖ¿å¤püÜ#¿å¡g÷¾œ¿à–hjU;ú¿Ñw-HrAGNbll@¡´9XPowerLawPMN J0019-8152?ïÿՏáVi>òö$Ç//€>õ8Û z>òö$Ç//€?ïʔ\T%?"Nä㛦?zµÑ¸`Ûj?"Nä㛦?ïôr|/Œœ?Xo3GãÁ?Wž'ƒ?Xo3GãÁ?ïÿ÷BÛá>ÄÑ™Wµ>ÑzL¨"Š>ÄÑ™Wµ?ïÿÞiy¸ >ô"fóÆñ>ðË@M!M>ô"fóÆñ?ï)—_¶'?³
,Ét™(?šÝÍx×'?³
,Ét™(?ïõ…qT½-?d+ê;aÇ?TõðÑ6Ý?d+ê;aÇ?ïÿ˜$D¬?¾ùôy?	öø
"«o?¾ùôyAGN3FGL J0019.1-5645@s{´?¢­?ÀMéE¿ý±qÀ:OÁä;~[À<mùÞý¿ä ìî¥{@;N	Î5@  €´ã¿ì;—"°BA¿Þ݊t¸Ž§¿ã'L]"H,¿ÑçeÈdeäAGNbcu@'¦éxÔþPowerLawPMN J0019-5641?ïÿ"ëšöÄ?ç2ÚèŠ?¢'?"¹?ç2ÚèŠ?ï͘é½Á?'(P¸"C?yp³o¤?Ê?'(P¸"C?ïÑVåb?xãØC+Ûq?wT|ÔÀ?xãØC+Ûq?ïÿ,´û>ûün—Ý›?´Î˜	À>>ûün—Ý›?ïþj:þ¦?19NNîø?)\MM#ä?19NNîø?ïD@Ç#?¯©!y5ù?—|÷íúÔN?¯©!y5ù?^×Á?Œ9̗'D?>û;ì?Œ9̗'D?ïúà
íó?;AÁ8+õQ?DÔÌ@È,?;AÁ8+õQAGN3FGL J0019.4+2021@\5ý~E€=ÀDð[ÿÛÀ:dZUÖÀ;ã]9–û¿áÕå
C@ñxô@ý1 6ç?ÚHtŸ|¿ë¢CgÄñr¿ÚESÔ	úL¿àû7Ê$Y"AGNbll@—çA [ÀPowerLawPKS 0017+200?ïÿ³Šå]>ül|,Sa?>Îxl7ç>ül|,Sa?ï×^­y9A?"TUUª´?tP©9‹¸?"TUUª´?ïÞãޔÓë?qTsÑß2a?pŽÄ´R•?qTsÑß2a?ïþøQœ(?4k݀S? zçrڃë?4k݀S?ïÿÑ;=æ>ô@"Z4è~>÷bNϒy>ô@"Z4è~?ïyaÄ|W{?˜»z¿ä±ñ?ÓÇpu¬?˜»z¿ä±ñ?ï»U4\?…‹Xäʑ?8»©Sï?…‹Xäʑ?ïù™…w¤?@Þ@â·Ä?K¹šé7£;?@Þ@â·ÄAGN3FGL J0021.6-6835@s01€
|[ÀH&a_–hÀ:J¾ò¶°À;ÿBûÅ¿â~Ž,öOŸ@–CPŒµ[@8B«v'¿äé©Cõg¿èÏÎ@F¿çú˜ž-8Y¿ïÿPÓP¹AGNbcu@€¥<ÓZ…ˆPowerLawPKS 0021-686?ïõ|T |s?[†sZ–S?UVĆyü?[†sZ–S?ïÌ ¾3Ø?'ßpB§'H?yïøŽX05?'ßpB§'H?ï4ÈÚ­h·?‡Ô_&üÐ?™fä¦ãM%?‡Ô_&üÐ?ïó֝AU?Eê[µ©¶Å?XRÅàJ‰5?Eê[µ©¶Å?ïúj¨¦?OGØ0Çy9?FU^A"6?OGØ0Çy9?ïé-;ޏ?±¦_²ýt´?œÚZ;ü)?±¦_²ýt´?ï
"ºÑ?"MŒÛ53?œ^¿V;á?"MŒÛ53?ïÙn_ž?jŸlR ?\dÎÄpH?jŸlR AGN3FGL J0021.6-2553@Dçڟô&®ÀTÎ]?á—_À9¼º"eÀ;Ζ67Ê¿ûõõuã\@$|>M@ËVß_Ìn¿å<RÐÝS¿Þ®îñËðë¿ÜR¤J«'"¿ã>"¤âD{AGNbll@—Á:û~'PowerLawCRATES J002132.55-255049.3?ïÿf\ÖDÆ?*?4eª1G8?*?ïÝÁÜPDÞ?dNé²½?qÌ.äé?dNé²½?ïï&.p‰^?a+®d@ï!?`Ùїµ²`?a+®d@ï!?ïÿù}ª>ȓOÑäÆ´>ÊxÖúµ>ȓOÑäÆ´?ïÿ$@"³?z8±98ü?wí
°i?z8±98ü?ï´±¼À? 
š—?ik€6? 
š—?ï×»<ÎßÄ?x€ç8¹P?t"aŽñ6?x€ç8¹P?ïÿ´ÛêL?'@œ÷
?ɺM?'@œ÷
AGN3FGL J0022.1-1855@Tû_ò®ßÀSØÊërªÀ98?±Æ·	À;NQ"GJA?ìˆÓY'Ž@ÞÊÏÇ~?üÈÇ>Ã_;?î¯ÎE.¨¿Ø.¬Ï¿ÐìBÅÿ坚ݼ^@AGNbll@¤».—OßPowerLaw1RXS J002209.2-185333?ïûËs?<ٙ~¶¨??CÒZ¾	ì?<ٙ~¶¨??ï·C™îå7?"eAyKš?'/…þ€P?"eAyKš?ïÎË?.9?tJ›
Èϗ?xš`o՛–?tJ›
Èϗ?ïD8{òi¿?xZ¤V+Ô?—xð†Ú2
?xZ¤V+Ô?ïô½•ˆy?U}h{^"?V"ÕmgC?U}h{^"?î俶!K?®µ%ö"×?¡´ÒæT?®µ%ö"×?ïƒå5àrØ?;ƒð­*/?²?;ƒð­*/?î`ù.æ¯?'1¯Vm–?©ÿ€l5®?'1¯Vm–AGN3FGL J0022.1-5141@s™ìºËCÀP4߀-·ÉÀ9'컝oÀ;®,nóÓ¢?áDÂé–~@Vál)?ÿ̅>õ!?Ô.¢)àú¿ÙݪƐ¿æR¢¢Ša¡¿Ð0žú'¾ðAGNbll@›_Ø­«ŸPowerLaw1RXS J002159.2-514028?ï÷Ö;iK?Qac£?PS‰R{Ý?Qac£?ïÒ]ŽA?‰ôíRS^ø?vÑ8ñPù6?‰ôíRS^ø?ïlƒˆ$"?ŽU揷?'oŽø
¿È?ŽU揷?ïÓiB¨Šè?`Fªw5?vK^±éØ?`Fªw5?ïÞ½W¹ÐF?re¹&?p¡Tk±E?re¹&?îà…1Çg?³A`Eۙ~?¡þǬ¢?³A`Eۙ~?înýöݹÑ?ŸJä9Vâ?© –oåã?ŸJä9Vâ?î‡,‡G‡~?š"ò­+þ©?§7ˆì$?š"ò­+þ©AGN3FGL J0022.5+0608@['¾‹ÁjÀL V·À8s¹NjÇÀ;:ÑY#‡Å?ì½Ã²œÊÑ@9aÜ>ò@–_¡PG¿Øÿçƒ~Ç~¿âœ§jŠò¿àjT7˜PL¿ãi,¶0BAGNbll@"Ʊ&éxÕPowerLawPKS 0019+058?ïÿ©ß?ž¯>ú#`Më‹?ˆ)ó–nÊ>ú#`Më‹?ïƆ–Ôå—?Š%1S9Vñ?|¼´ŸÜ<?Š%1S9Vñ?ïÕtåôÕÄ?w*òÎ
?uEŒþùò?w*òÎ
?ïq¤0‡˜v?o›ÙY1þ`?'ËyíU#5?o›ÙY1þ`?ïÿA~¥w?~ŠÂ2?й_¢¼?~ŠÂ2?ï"ñ`nÄ?ªÑ'øHY>?Ÿ›¡ÚÑ_h?ªÑ'øHY>?ï½Ø{ŠB—?"žyx^?€‰áŸæ:?"žyx^?í«ö{/v?—Ü
£³#?² O븐Ï?—Ü
£³#AGN3FGL J0023.4+0923@[Ý? §?ÀJmÎÿ¬óéÀ9¥:¿ïn¸À;×Ájî‹?ûðT5:Ÿ@ƒ`–mÀ"?øbÀú†™b?µ±¬lÒ]¨¿âç·¬ §7¿ìÒÈ'²²«¿ç…¨á$PSRPSR@ŒF!…ÆPLExpCutoffPSR J0023+0923?ì¨ÍØÕ3?Á½­:
?¿â¹'9Vk?Á½­:
?Ñn7vAƒ?Î1^-"?çHÀdDß>?Î1^-"?åHº…'=Ä?µ†œ7¥?ÕnŠô݄w?µ†œ7¥?ӚÕ|QgÚ?­ŸÑý7?æ2•A×L?­ŸÑý7?àù¦J¾%{?ͽE²´?Þ³jƒµ	?ͽE²´?ºº¾öSž?ÆmÝ~ëƒ?쨨!5žŒ?ÆmÝ~ëƒ?ãòýV¾ŽØ?·± Ìоú?ØR'âQ?·± Ìоú?¥¥j©'-?œbiT3?_ãÍ?œbiT3MIXED3FGL J0023.5+4454@]oâއ	tÀ1¯X?\6bÀ9 Q¯<ÜÀ;¼fÉbµ¿õ°¸´çÓ¹@ú@'7|n@ŒF JÎ/¿çôª}±J¿å´³5ˆ¿è¿`ÉLc¿å¿½Ù{4AGNfsrq@ƒc¬q³PowerLawB3 0020+446?ïþõ{9(¸? Ì­ó‰H? ¨PSÏǛ? Ì­ó‰H?ïæ­u»æ?"m,ƒ°h?~,©CHâ?"m,ƒ°h?ïä2îßW?^–ú£ŒÆÿ?kÍãQ¹P,?^–ú£ŒÆÿ?ïÿÅ>|×0>ô´­‰ß‰>ý`ijvW>ô´­‰ß‰?ïý!Òi§?8».ÃfÿÒ?6ñm£}¡ê?8».ÃfÿÒ?ï5ì`äi?¤séáÏv?™BsåLlâ?¤séáÏv?ïÀÜM7/0?|¼+9˚÷?'ÙZ"
?|¼+9˚÷?ïúÆC,
Ü?Bˆò.Š?DæóeERà?Bˆò.ŠAGN3FGL J0023.9-7203@s©_ªŠƒÀFs¡€èTÀ8^½ÇvK·À;f-ù7Žã@¶@)æ®J@ø	24?ö"»J}¿µtDJ‡¸œ¿ÛÍ:°ÕöA¿æš*ž9;‹¿î#J]'OTHERglc@ŠÃ}¿H€LogParabola47 Tuc?­^¼6?%µå‰.pO?ïÿJ"ès¶?%µå‰.pO?·n=Z9?ǃȖ9ñ?í?x™wh?ǃȖ9ñ?¡.0È}ed?—s¦.Â$?îíóx)ª?—s¦.Â$?tš8¦ë¶Ð?_GP»H.Ý?ïÖˎçÂz?_GP»H.Ý?F&è7nV?B‰ W^
?ïúvE×z¦?B‰ W^
?©EÉ*.fk?¼pÇA·IG?îk£m"Y?¼pÇA·IG?Ö#© »?‰9üuèמ?sÌÖ]?‰9üuèמ?=[ýHF?4dž¯ô§Í?ïüTŸi'@?4dž¯ô§ÍPSR3FGL J0024.4+0350@[M–ÃüÀM,Úÿ•võÀ:Þ
ò}À;¾Êe€?ðAUÈ3‹@DpýC77@9ÎÀ—à1¿àëÝ3L]§¿æ¼,ÆÝt¿ç¼æç;t1¿åÀ|µ2AGNfsrq@'©ZÔ,<ŸPowerLawGB6 J0024+0349?ïý
ÞK5š?GB2Ã"ϳ?7'û擼?GB2Ã"ϳ?ï¸ðüÜê?ýGz#Bá?ÃÀüu'?ýGz#Bá?ïªA½9±Ò?ƒÜä&¦?…o®#ïg?ƒÜä&¦?ï4^Éì¦?xû+ÚwMö?™t?Yq-?xû+ÚwMö?ïúšÊ_ùÕ?LãƒÆóö?E"Ö'Ø]â?LãƒÆóö?íëŽnmEÿ?ºú®Ô¶ƒ?°£ŒË?ºú®Ô¶ƒ?îÐí%æL-?›t>$Ú©?¢ñ-¢w$)?›t>$Ú©?ë]›˜¯]?©O™Ó¿v?‰'ŸáBŒ?©O™Ó¿vAGN3FGL J0025.7+6404@^@¿ã°?õgq¡-ÒÀ9Ë/þËLšÀ;5í£ùo¿À¤®'À•@Œ-ëÉ@±§¶Cž?ëÿ&ò³¿çú
½'×á¿æ;×F£R¿Åoúä¸%÷OTHERsnr@«}ZáG®PowerLawTycho?fdÍMë?­+* ÷»?€žf¼.e_?­+* ÷»?ﳊ¸o•?'0^Ýÿü¯?ƒQó³X—?'0^Ýÿü¯?ï<ěýï?'Ðò)ex?˜guH
?'Ðò)ex?ïôZZòó[?G PT£oŠ?WKJÊ·?G PT£oŠ?ï|¹9Ù?™ï›Ž#_O?<(ØÄÛ?™ï›Ž#_O?î-
üùT?º
°þÌ4ˆ?­/_ÏTƒ¾?º
°þÌ4ˆ?íÅP­?§Ü4q<Ql?±Ôø‡?§Ü4q<Ql?ïX»cK‡p?'$æS?"è""uõ?'$æSAGN3FGL J0026.7-4603@s½¿ "`ÀQœˆô'À:'–Æ€'qÀ<é¾u5¿ð¹1ø¶Õ@)v'hO @šK`%¯'¿â·4¶&Sb¿é'JO¯j¼¿Þú†¡øÁP¿è.4v)R	AGNbll@ü@ŽÉPowerLaw1RXS J002636.3-460101?ïÿAù–ü©?ë脓7?Àχ´P`?ë脓7?ïÒŸ³ÓÆ?Œaõïøú?vö0yµ?Œaõïøú?ïãYÇz0%?cÈ!"ŒÝô?l¦8uQº­?cÈ!"ŒÝô?ïÿˆd¤*¨>ûñùc·YG?
æÜàçÆ>ûñùc·YG?ïÿ­ǜ?LF# [6?ºöhn?LF# [6?ï8ç3´¿?²§%À
_?˜ã¤È 
?²§%À
_?ïÑ+F³KO?v–i¼Ô%?wj\ Úø?v–i¼Ô%?ïúA³Ë ??©Æ!­?Fù1©/Ê<??©Æ!­AGN3FGL J0028.6+7507@^[òà\̊@( Q¿æ4}À9µ´v"±ÓÀ;™Ž"¬Ï¿ìº+­Wçs@
~kjÝ@»M DC&¿æG9H‡>‰¿ãÄ`óhu"¿Ü`†ÜX¿îÈ·ôoöTAGNbcu@'SÁ×ÛôˆPowerLawGB6 J0028+7506?î Ö#ÃK?¨€Á-ø¯Ö?¥òŸË0S?¨€Á-ø¯Ö?ïÏ-œ'¿­?†§v—…?xi1ªA'?†§v—…?í‹p»Ì@Ø?ŸÂÔf-¸?³¤z!0¿?ŸÂÔf-¸?ïöÎÕg®?C‹çÀ£?RbU'aóQ?C‹çÀ£?ë'¯€?¾jh·³?Á÷éCƒ–?¾jh·³?îÎÒ73·¬?¶âá˜(.?£܎|S9?¶âá˜(.?骴ZKa9?³3*½­oñ?ÉU.–Ò{?³3*½­oñ?ïMp额?lz7å°°?–QâƕBu?lz7å°°AGN3FGL J0028.8+1951@\ë°À&ÌÀEYÝà‡kÀ9üaCöÈÀ;Ë«Ä>ˆÒ?åÉoïxð@šÀ`-@x+ßVè¿æ‹ƒˆ±¿à›º%'p¿î°-ʓŒ?¢MLu4ƗAGNbcu@‡ÎCa@OPowerLawTXS 0025+197?ïù;»Ë¦?Z;Ùldυ?K"þ­Ì?Z;Ùldυ?ïƃ¤‡*Ï?'§ba1?|¾-Éy­?'§ba1?ïUª`³–g?ŠJÛgç'B?•J³â­û?ŠJÛgç'B?ïµöÍ?vU¿Ó&ǂ?'¹>
‹Îó?vU¿Ó&ǂ?ïº@'QÓ?‹™Ycæ²¼?oÛ½#	6?‹™Ycæ²¼?îWRB½¾?³ó%'ŠŸ?ªŠÛÜLV!?³ó%'ŠŸ?ìØS}u?¨}жø``?¹=dZ&?¨}жø``?ëCЯ…i6?¾…ŽÆhø?Âð½Aê[(?¾…ŽÆhøAGN3FGL J0029.1-7045@sKÀ]RÁÀG!?©c;À9Žslf×À;ÂDw(UŠ¿ß:]¦Ã@>-_‰¨`@F±_ˆü"¿èm:$¶e$¿áBf=1ö¿à!Ô³mx¿çbN°«ó¨AGNbll@"¦9#¢œxPowerLawPKS 0026-710?ïýú"ôy˜?,Ûd·L?0+×ːu?,Ûd·L?ïÕ"ېù§?ˆ9>¡9?un'4Ã|§?ˆ9>¡9?ïã_fv?k>/W/ã…?l ôWÜZ?k>/W/ã…?ïüø.'ýÔ?&rÓD"¬?8>‹"'Þ?&rÓD"¬?ïúת zt?Fz"ÙN?D¡WׄN?Fz"ÙN?ï+£tWÐ?¯½ÇÇÓL?š‹'†4=ó?¯½ÇÇÓL?ï¨ÄŠ3<?‰e¯Í±¥ß?…ÎÝb
%?‰e¯Í±¥ß?ïáÉQÔDL?a¿Ãò'Ý?n6®IøD;?a¿Ãò'ÝAGN3FGL J0030.2-1646@X!T€uÀS¢î «†À:ÆÌ؋GÀ;Ôač?Òd
VæÓ@§rëZ§?úZê:GÏ¿ïœ Rc'º?ïÿ™¤ðÿv¿×mÓôv¿Úbêc",¦AGNbcu@³ª	ã½PowerLaw1RXS J003019.6-164723?ïÿ®ÃIJÄ>ûŸÓǗkÖ?OТ¿>ûŸÓǗkÖ?ï֋««{*?‰0@µ]â?tº*4'??‰0@µ]â?ïê«>ª=?jݽž{<¢?eTÁ'wâs?jݽž{<¢?ïô1ñê"?E¯¨.ƒlá?W㛣8™š?E¯¨.ƒlá?ïÿ¶kXàä?.nEžÜÿ?eÉEe?.nEžÜÿ?ïcH_üP.?AQës?"–ô-È3?AQës?ïåÊO¢ˆ3?w_m釁‹?j5°<{Œå?w_m釁‹?ïÓðÞá¨?it=•:ýë?vªI?it=•:ýëAGN3FGL J0030.3-4223@sÔÖàL'ÀRˆð€0<À8¥§
›duÀ;¼^¸; ?ÚJ"Õߒo@‰«Ó
@¤ë€—.¿åÚÎÙ¨Ž¿æÒhõk¿é•";
ºf¿çí)]5TAGNfsrq@yô—ÿCBPowerLawPKS 0027-426?ïþü
=fy?'øKX°? ?*
oË?'øKX°?ïÌ
R‹µ?ð·¬Œâè?yüúëWÍ(?ð·¬Œâè?ïÎ.¸,à?nÕxõgq?xòh¹çÄ?nÕxõgq?ïî'%÷E?Kiê<0~?aØÚæ*ÂÒ?Kiê<0~?ïýá^̋?0œª†¥×?0õ1æµC?0œª†¥×?ï*OÈíT?±çf|	1?š¶÷:ë?±çf|	1?Žå-
?…±wW?‹ÜJ$X¨?…±wW?ï|šSd^?'¾¥'ÒTf?lµœÚ>?'¾¥'ÒTfAGN3FGL J0030.4+0451@\Ie¶™…ÀL͵_ȽtÀ7††*QbÀ;8k)«@­ï`J˜€@:֑ó?ÿ,-Z+¿Á7#§=àпÞ°NxR¿çîßNã¿î&Çy­¦PSRPSR@‡Â"¼PLExpCutoffPSR J0030+0451?Q…èN•ß°?Vv4c®¬?ï÷=¬º?Vv4c®¬?´Yē–•ñ?Åå²l·?ítÇmšë²?Åå²l·?¨Þ­¸®9?Ÿ¹,"°/?îr.˜ø=?Ÿ¹,"°/?I'šÈø?9ë]CÍF?ïù¾ßh¼?9ë]CÍF?YHÅ'?Sja=tº?ïór[š¹?Sja=tº?­›ÃjÉP?ƞÓráÒ?î&CÏ@M+?ƞÓráÒ?œ"€ç,Z¸?ž$C?ë‰n?ï[øƝ*?ž$C?ë‰n? VçD"?lY\úK?ïþö*Dzd?lY\úKPSR3FGL J0030.7-0209@[¶ýŸÓo~ÀP"Ñ¿æ4}À95eWr­À;­7Ÿ©~?òJß³õ:@qa²øe@V_]2¶¿âo58WE¿åÍKaA'V¿æI×é2¿ïÿÒXÛlAGNbcu@…Ŧµ(PowerLawPKS B0027-024?ïüŸ–¢ˆ?;è#Ǻƒò?;ó(v®÷?;è#Ǻƒò?ïÔ"vÍfÑ?…Aþ'»µÀ?uîĕÜû¸?…Aþ'»µÀ?ï2SŒ'j?‰®§Dhj?™µŽz~6Â?‰®§Dhj?ïë¬à.œ?Iö¢Õ–æÕ?dS™Ì©?Iö¢Õ–æÕ?ïûˆ7­§?Cð«í†j?Aß"#ˆ?Cð«í†j?ïFxU.ä"?«÷~_à¡?—0õ[ÛIÈ?«÷~_à¡?î"|e+S?Â! ?¦¿88ÑcÓ?Â! ?ïӗ3ã²B?i"{-ºüª?v4f§E?i"{-ºüªAGN3FGL J0031.3+0724@\ŒÿyÈCÀKŽÃ€ðÒÀ: &yÀ;Øöfú
?­òw7aC¦@ù䥆ŒÍ?ý.µÀ@ÍP¿îǨ )z?ëêDE:'ï¿èS´t³¨†?È®?-'_iAGNbcu@±©ƒn˜PowerLawNVSS J003119+072456?ïû"ÔN3?Y$îÜ÷ÿ?A찄»ê?Y$îÜ÷ÿ?ïÆþ\?"@;'#ïÎ?|ðûùàª?"@;'#ïÎ?ï~±ˆ›
?…ÞóJLðÃ?)Îçvt»?…ÞóJLðÃ?ïø£÷…Kô?A²›RýË?Mp!/X¶?A²›RýË?ïótÂRS?V©ŠŸv"?Y{•L_?V©ŠŸv"?ï´<T't?µÌݏxê‰?Ÿ‰x~×o?µÌݏxê‰?îÿ9{̪?":ܟӚq? hBYwÞ?":ܟӚq?‡Z>?Œé`p¾.?ŒÒÞ2œs?Œé`p¾.AGN3FGL J0032.3-2852@"Œ¼ÀO(ÀU\>ÏuÀ:®1ËT&ÉÀ<âP3ÀÌUàÝ%
@
²gEß]@"! 
Ñû¿Ö{ãaÈ¿æ
8$1Ë¿á¤û|§_¿Ù'ÈÇQLAGNbll@™¹l¿±[WPowerLawPMN J0032-2849?ïý@AS?DØVã¥x?7Eþœ:¤:?DØVã¥x?ïÙ¿¢Óæ-?l$£$[?s .°ÙÝp?l$£$[?ïN¼›Ò.?"]¯µiù?–(l‰)Ú¦?"]¯µiù?ïÿÿþc®â>Dhc¹"ìÀ>(§ur‹#ö>Dhc¹(•?ïò7œhDÒ?bÐpăë?[Ç¹,Â?bÐpăë?ïhˆÞ$?œ" t¦Ü?‹åÝÁ›ÿ?œ" t¦Ü?îLî"æg†?£YO9EÎ?«1Ïá¹ ?£YO9EÎ?ïÿÿ"T×>£ Ú#>É>‹'´÷ÚX>£ Ú#>ÉAGN3FGL J0033.6-1921@W'¿ö$µÀTNW_ÍÅñÀ84©Tø€À:¯8hýœ?æócm_Á@¬¡fítã?ûo yÒ¿Þ¢þIh÷¿ÔÖhW¿Óëm"ΠڿÖù`ïYÂAGNbll@¢¼CS&PowerLawKUV 00311-1938?ïø5H-¹?LhdD¦?O£**j{j?LhdD¦?ï˛̈́
o?‹J³d¤3?z2M…?‹J³d¤3?ïk÷$d8d?'`')!{??'v菂?'`')!{??ﱱДyì?n4ì€ý,š?ƒ"‹ãxŠÖ?n4ì€ý,š?ïñ…‰i¤?_Z¹ŽÉ]_?\ôî-âgÇ?_Z¹ŽÉ]_?ïA- ?ª–d.H€?žÜÓp¤?ª–d.H€?ï6גÍ?˜hÊèYE?™%
À,âS?˜hÊèYE?îåoW?›»?ŽÍ—ÑWû?¡©
ˆ–¨S?ŽÍ—ÑWûAGN3FGL J0034.3-0534@[ß.ßç[ÄÀQº¿ïn¸À8½bð À;›ìVuX?þÍæ°M»@æ`pX,½@%G—ÙW'휿ٿáÕ`•Ó!·¿æA†û‡Jb¿î¨ö4­ºPSRPSR@…åí'hr°PLExpCutoffPSR J0034-0534?`èWðgh½?kƒµ˜Ò?ïï¨XG?kƒµ˜Ò?¾/³%J¬?ʯ™å]¬?ì:	›Vª~?ʯ™å]¬?ÊÒtûï>?°–Bƒ$˜?éKbÁ0€?°–Bƒ$˜?¨)ȝ17?™~üZŒ?î}n?3-?™~üZŒ?dÓ]­«¯|?g¥QHs•?ïë,¢†Ž`?g¥QHs•?¶×º†Ï¡?ÈáÜÚÈN?í%¯jÕü?ÈáÜÚÈN?Ǽ^ÜjŠÊ?±mRÇUÈ?êèHå]N?±mRÇUÈ?y=º=¦?kä;Nð³ô?ï̈́‹H%¼?kä;Nð³ôPSR3FGL J0035.2+1513@]IP?³t6ÀG»ÒàD²À9OíhMÇÀ;P"Ý?à|[jVWr@¸e{.õa?üç€bæÕ¿ãÓ5»4P¿Ä¯Wíó¯¿ÚCRóà¿ÖEˆ–£+OAGNbll@¨½'Zîc PowerLawRX J0035.2+1515?ïýjö‡Êÿ?-–§ B?4¨KON£_?-–§ B?ïÕDŽ…Ø"?ƒJ=¨7…=?u=Þ¿áÕ?ƒJ=¨7…=?ïÙÛo'f?hóOc?s|h‹ ±?hóOc?ïÒY.˜Ø?W¼²9)í'?vÓiðô?W¼²9)í'?ï÷
ˆSÌ?K¦Íu¥6£?Qäï|#å×?K¦Íu¥6£?ï:¾©Ö?²æYo­Ãå?ŸØ¨0ï8?²æYo­Ãå?ïŽ,Ð1u?‹A^ñ²GV?ŒtËýñ'<?‹A^ñ²GV?ï	ã¹ÖÙt?…yñ ¦/(?žÃˆ¾E™"?…yñ ¦/(AGN3FGL J0035.9+5949@^?ßÖkÀÙß`£-íÀ83J‰'
ÚÀ:õWÁ‡õ,¿ÌçSÐ{qÕ@÷Õ±Lé"?þ]I^î¢à¿Ó}•?uil¿äÔîuOH¤¿Õò™ûiBd¿×á&$AGNbll@§/-à
qPowerLaw1ES 0033+595?ïýncÇ
ý?19a"'k?4ŒàLS9<?19a"'k?ï¹íb¢?Œ'"|P?¾D­Þ¼æ?Œ'"|P?ï»Ô Ësÿ?"\ŠUÀ0?
÷½¬Âm?"\ŠUÀ0?ïühõse?(ΒÉ,?<¸UåÎ"?(ΒÉ,?ïùÁòÿ?O€¬ïQþñ?K˜ù
k\{?O€¬ïQþñ?îs¦•Ö?»ŽnWÌo°?®HÇNp—?»ŽnWÌo°?ï°ùRol'?ˆEç'óN?ƒÁ«]´@?ˆEç'óN?ïç#U3}?a)—M˜õê?hÿܘî‹%?a)—M˜õêAGN3FGL J0037.9+1239@]r7`¿]yÀI
Ô¿àU@À9PäEVÀ;ŠG?¿ÕKÐõ%†@Èé¬+—ˆ@6<6[²¿â	ÚIb¿å¶ì"çʙ¿ÝÂÈïiý¿ã&ã
?¸ÁAGNbll@•®µ%F
¦PowerLawNVSS J003750+123818?ïÿb48Òì?Ã-0Bº?¹u?îd?Ã-0Bº?ïΓý+?Žð)'©'¿?x¶W6©P?Žð)'©'¿?ïóÔü,ì?agc¤²¬Ü?XVx¥â¶ò?agc¤²¬Ü?ïüD¾9ÐË?(Ž¥ßP?=Ú
:ɘ?(Ž¥ßP?ïÿŸ4¹=?;Z¹DÇ?2Ô9Ë«G?;Z¹DÇ?ïcþ	H?§€•eÓ$?"€. •Dø?§€•eÓ$?ïë!Ω=H?uKmFimÅ?dÞ1h ¯æ?uKmFimÅ?ïâ³áÄU°?`WZ.
?mLoY?`WZ.
AGN3FGL J0038.0-2501@PÂê /JpÀU•IÿþRÀ9ÀF¯ç¹¸À;á"Év7?ãLL@µ>@«õ–?G@'ã@V²>¿åkñ&!U¿å|CåÝê׿ç¤NyhT¿ìÁ‡§Ý2AGNfsrq@†îCÞ灄PowerLawPKS 0035-252?ïý…os³ß?5üÑ…|?3ԂAm¾?5üÑ…|?ïȊ4Îû?'˹7ªÍZ?{ºþ`"—?'˹7ªÍZ?ï¤VÏ£†?'¬‹f;Ø?†êLY&}?'¬‹f;Ø?ïÇ÷Û¢?^ Æaâ<Ý?|ur‡Ë?^ Æaâ<Ý?ïü¡ŠÃ¹?Aø}½ã€d?:óªƒ`?Aø}½ã€d?ï.Ó@j|?¥í6æñç?š%—ðöB?¥í6æñç?ï˜F"×£ô?‡['Å¡`?‰îwM†Ÿ?‡['Å¡`?âê­?‹Í-cÉ%?¥D‡9?‹Í-cÉ%AGN3FGL J0038.0+0012@\ì  ô×®ÀO<¾Ÿã_¶À:[¯ˆïÀ;Õ
»ªeš¿×:]ã¤Ä@'QS"·@@›àEÐo¿Ör:ˆD»$¿æì•^ÃÒ¿Õ"˜Ue§¿åXNRÉP–AGNbll@˜8—Á½¥PowerLawNVSS J003808+001336?ïÿf}›?L¯ L?0[ëÑC?L¯ L?ïÏømm?òÌá{¢¼?xuÒ8l¼?òÌá{¢¼?ïÜÖÐå=å?g¸¦£?q"—t£Ýj?g¸¦£?ïîÛ2Põ?K9™ªd°Â?a$Íínºì?K9™ªd°Â?ïþöHØG;?!Qûm´=? ›s0?!Qûm´=?ï-á¯ÝÓ°?°ò Clf[?šCÉû®"?°ò Clf[?ïĵ_%ˆ?êp÷ŽíC?}¥PL?¾ó?êp÷ŽíC?ïP§ï?ˆ\ß?pLQ?•ðzS4.?ˆ\ß?pLQAGN3FGL J0039.0-2218@VúQ?ùSÀUp¿ñ7À:ÊËi~KÀ;çåPQQ+?ï¡¿#R%Î@Ë+1¥?ûr"^úŒN?îÚ²ämà¿ág5离¿Ë3^ÿ6Mç¿àÆ<¥ÖF|AGNbcu@³¼–âëCPowerLawPMN J0039-2220?ïùøD}f?EŒÈîéÂ?HíF$x?EŒÈîéÂ?ïrFéjߔ? Æ¡®öT?'·"Ö©r? Æ¡®öT?ïy>˜6Î?‡šÇAªÜ?Ø-`5?‡šÇAªÜ?îÌE88<?‰ël—zR?£;¯ì<?‰ël—zR?ïú™ïÞRd?D4&
ƒV?E˜?§ƒ?D4&
ƒV?ì@-©ÓÅÝ?ÆB¢ÀéÑ?½þ'±aÑ?ÆB¢ÀéÑ?ï¨À9QÁ?•Ñ±]}?ŸÊçñöÚ?•Ñ±]}?ìµoz®"J?§ªFãYÐ-?ºT"*‹]°?§ªFãYÐ-AGN3FGL J0039.1-0939@\:'@·€4ÀRŠ4fÀ:E$oKvÀ;ß¹Z)AB?í"Ìû=@´¶|ï@ÀsÀ—	q¿ÚR)³W°Á¿êº"vØà"¿í›RÙw¿ïý_"î—«AGNfsrq@Å A‰7LPowerLawTXS 0036-099?ïÈ#îzO/?ƒQZož¸?{î¬Úè'?ƒQZož¸?ìwØmƒªß?¿ô!m–?¼A<"â©?¿ô!m–?îG
ÔLüf?šŒJ"Nc¯?«R¸œ"ª?šŒJ"Nc¯?èàŒó?¦>ì=Å!L?Ì}Ì3Ÿ¿£?¦>ì=Å!L?ï®HF"ˆ?Œô	×¹¾?"mîOj+?Œô	×¹¾?ޙÌd
—?ҟVïS°?à³ͱy4?ҟVïS°?ëì䵪Nü?¯<‹È0ìî?ÀLm)VÄ?¯<‹È0ìî?Êܜc"!?¯—¼­Bq?éHØç7\8?¯—¼­BqMIXED3FGL J0039.1+4330@^%~0‡‡À3PlÀ»"À:Mq
"À;àÎs•ùÒ?㽝lb@Šz¥7²t?ÿgîÿQ¯J¿éD ±³8¿Á'cÿj¿áÔ?®#ȿݘҔŒê_AGNbcu@¥'"h	ÕPowerLawNVSS J003907+433015?ïþO˜»ð~?)ƋfÍé?+s\ETÜ?)ƋfÍé?ï†<nŸÉ?–1H-ˆ|Ð?Žp䆷E¥?–1H-ˆ|Ð?ïÝɾò»ì?`µí¯'̘?q ¢éÉ?`µí¯'̘?ï"]®m!?þpGã†ß?ŸïtM¡÷Ì?þpGã†ß?ïõA¾qg?Sµ'g+ùO?U|"]ŽÐº?Sµ'g+ùO?êØí$Ž³??Ä®F¶ô?ĜKmÅ3?Ä®F¶ô?ï"CÄGe?ˆ^-z$[?‹?¯ 2Ä?ˆ^-z$[?èì
¢Û?³-ï³
?ÏôOÕw¸–?³-ï³
AGN3FGL J0040.3+4049@^*§"X¼À6J_Ÿ¢ÈÀ:³t«£‡YÀ;³6nQs?ÔuüÎ-†@HG§‰qX?òºÀۧܿç@ÈôfL¿èXBd‡Æ¿Ùîh§Íþ•?Ôð3ásAGNbcu@â*?
=p¤PowerLawB3 0037+405?ïý
[Hó?PÿÍR­?7—e]˞q?PÿÍR­?ïÆ·'ä?'CUØ39<?|¤t'už?'CUØ39<?í°¦=Á×{?§ÚzrR{û?²zΧi§?§ÚzrR{û?ïüoÏh*?1Œl4ß?<'šéð?1Œl4ß?ïüI+rF?A,ô5?=¶¡"Œ›F?A,ô5?îî"¢Â7H?®¢3.÷&w?¡ÕÑH֊?®¢3.÷&w?ïvÁ»ªC>?ý£¶&bØ?''ȅ.S?ý£¶&bØ?ïÕRE®F5?wZkŒ8-©?uVÝ&5o?wZkŒ8-©AGN3FGL J0040.5-2339@UÊá`ÈWÀUoÌþ£	À:ߍ'ûÀ<ϗ'h%?Ô½
˜Æq$@,҃Åò¾?ÿ#¹€iÇÅ?ïŒp3:a¿äX­šúº¿ä77	¯¨¿¦"ãæ*',AGNbcu@§†Ç®záPowerLawPMN J0040-2340?ïÿ3¾b?ª?$Ÿ<"_\œ?ˆ90Ô÷?$Ÿ<"_\œ?ïÌü®¢üU?‹'mÝ*÷?y¨º0j?‹'mÝ*÷?ï™5 m?Á?‡ôS%KPý?‰²—òn·?‡ôS%KPý?ïúšhª?7¡×–ЗÐ?E–]W§Y?7¡×–ЗÐ?ïÿh%¶Ñk?˜—ÇÉAj?ûAÊ#£1?˜—ÇÉAj?ïdR½ZÐ?§uVäÖ=?"u¿¦œØ?§uVäÖ=?ïa·CèPü?'æ(ÅDbó?"É'õà?'æ(ÅDbó?ïÞÜç¢6?k†ý­Ã'?p'ŒOô$ü?k†ý­Ã'AGN3FGL J0041.9+3639@^4´A»Œ3À:+ä€G¸üÀ:»•EwÀ;÷ÇúÕô"ÀñçßÃ@bg¦'`B?ÿœ»úl?ïþÁVw¿î7à†4¿Å#»L'ö¦?¤»ùë¾ÕhAGNbll@«ºmÅÖ8†PowerLawRX J0042.0+3641?ïÿXÑߗ?j¶?ýGûÖÀÑ?j¶?ïÔв"T?…a}ôL˜Š?u—¦Ë~?…a}ôL˜Š?ï¸ ò'­´?'ìvK?÷Ã\ìÙ?'ìvK?ïÿÿv$>œµË¯¾>+yâ£
>œµË¯¾?ïÿ[…óÜ?*³õŒ"±7?Ԕ^lþ?*³õŒ"±7?ï0w)ŠÆv?±ó
B±Ó?™ñÐ^ÿI?±ó
B±Ó?ï­döQ?"Zj(#?"¸çÀÛ¾?"Zj(#?ïÿóô6¦¹>äÉê†Ý>Ø XtŠd>äÉê†ÝAGN3FGL J0042.0+2318@^	F^‰"SÀCÂߥ¥À:‹ ²'À;Ð:‰hÊ?ØÄ·omv%@¥¥À‰d@Õݟ­ÚÄ¿âxj
K(Y¿ç<4–,8¿àn–
ÃÓ¿ïÿÄ^œÌAGNfsrq@÷ÚQÎPowerLawPKS 0039+230?ïþlªMF?'켍.K?)5YP¢[?'켍.K?ïÀ ~z?†ë¥VÆs2?÷p-ÞÁ?†ë¥VÆs2?ïl›ž£æò?€ÉÚU~¾?'lŒ2bY»?€ÉÚU~¾?ïBu?ƒ?v&¢vûF?—±X%{§¦?v&¢vûF?ïþWÀ—,?4iª­‹ÆQ?*ƒüã%"A?4iª­‹ÆQ?pJ¯•?¯ní 8áq?¦çXúyª?¯ní 8áq?îÐP}Põ?™v˜4U!d?¢úþ©â¾±?™v˜4U!d?꽸/º`l?®"Ì*4?Å	A~O?®"Ì*4AGN3FGL J0042.5+4117@^He¶™…À5‹x_.QÀ9ÛÌ`–BÍÀ;Ç6oþ•?ãˆ=ZmM¥@
kzÜÀ
@¥ŸŒLտṙaܔ¿âÛ
½Wäÿí7ž­)Ä¿âæa(9.OTHERgal@æ>aÏþ°PowerLawM31?ïïnÃ_Ä?uúY¥FL?`ÿ'9à‹Å?uúY¥FL?ïFÏêÈ?žöFç?—-æ»=?žöFç?ï`Ý9pRè?ˆ÷¡P‹ø`?"äXÑõ¢ü?ˆ÷¡P‹ø`?í×сM®›?'šuÖ?±AsöÜe¨?'šuÖ?î*ˆ`¥öä?µ?Ȗ'l?­Wyõ 'Â?µ?Ȗ'l?抏Y¾|?ÎÑ,9ç#Ý?ÒêáLƒÔ?ÎÑ,9ç#Ý?ì÷àÕJþ4?¨Û†<ßH>?¸@ùTÌ'd?¨Û†<ßH>?ܗ!ëÉMx?Á	÷¸çER?á´o
YD?Á	÷¸çERMIXED3FGL J0043.5-0444@]rö@c^ÀPâŸÞW9À:‰¤f|5ÜÀ;Èà¨KäÀ
ÉlüX@
'¹Özök?ûÀÝ "šY¿ì5aËÞ!¿Òƒw³¼½¿Ð´
¤¿x¸¿Æ±
3oC/AGNbcu@¹\$?åÉPowerLaw1RXS J004333.7-044257?ïÿQUqw?Áü¥—ì?ÕUÜü¥?Áü¥—ì?ïÙàˆ/RÃ?ƒ¥Úþ:nk?s»ð•®š?ƒ¥Úþ:nk?ïÙmç~æ?xÆ¿|¸#|?sIu—ï8õ?xÆ¿|¸#|?ïÿÿþíA>&¯4":'>#@ÿ¾ÈûG>&¯3K=?ïÿÜò4?¸V"å–?¤fZ?¸V"å–?ï[ÀOÓ?­‹ÛP•ê?"‡ýo>í ?­‹ÛP•ê?ïÚ5ùa*g?wóYùÐvà?rå:8o?wóYùÐvà?ïÿÿԃqÜ>‹<Ëٖ%>uÝz"¡ª>‹<Ëٖ%AGN3FGL J0043.7-1117@]žYò»ÀRƒ¢ÿßHÐÀ:O".bêÀ;r²¥Z?ç÷ lÿT+@
Aï8²?ùæÀ
¿ïþÏA­Z¨?ïú˜G£Ç¿Ò±á3·¥¿×‰ùÉ/3tAGNbcu@·'Ýp£×
PowerLaw1RXS J004349.3-111612?ïþËݎý?Å2ati‡?#B)¬Ø!?Å2ati‡?ïtߨX?˜B»/y;ì?'dÖJþ?˜B»/y;ì?ïËwºC)Ã?y¢i"Þ­?zD"ǽ²À?y¢i"Þ­?îgökה|?ÓúSó¼?©€™D>†>?ÓúSó¼?ïýh¤6ß?1CÿI•Dl?4ºßVhŸ­?1CÿI•Dl?êÖUÃg.Ÿ?ÈW$ÒÐÐp?Ħ¨òcE†?ÈW$ÒÐÐp?ï‹ú±Ùε?‡
ª—Ö'k?Sx^FÃ?‡
ª—Ö'k?éL%;½Š(?±ÀÚ0¿?ÊÏk	×^?±ÀÚ0¿AGN3FGL J0043.8+3425@^J:>À/0À<j'_8t¼À8¾Ž'b™À;Xó"
3¿íÓ>Bä_@žŽ5	L@[ŠI{õ¿Û¬š%8Q^¿ãʽ ßÞø¿ÚxÈՂ¿ã%NŽáã=AGNfsrq@–b‹]ÌcñPowerLawGB6 J0043+3426?ïÿъ²Ý>îÑH•}½>÷:´mÉ.ö>îÑH•}½?ïΫf{y?ŠK.RÔ?xª~æßKk?ŠK.RÔ?ïðOüA¯x?Oá"]Q?_`òӟ·?Oá"]Q?ïÿÐÆ!–>ힲk˜²&>÷ðEÖ#>ힲk˜²&?ïÿÌ"¥=ß>ôO	Iv">ùîΕ›Öõ>ôO	Iv"?ïK…¹à-t?«X-¢&eW?–HŲy?«X-¢&eW?ïñÏ}<}?e"Þìƒz4?]è`ìÉÖD?e"Þìƒz4?ïþšÃ[?"£ÀÃV?&WãöBêœ?"£ÀÃVAGN3FGL J0045.2-3704@s`—ÿ›V2ÀSý£¿ø¨ôÀ9x/Äé©|À;êöÃ@\¿ää†Ê+@¡aÈ
þ@Wºßd¿åþóX¿ç'¨²¢eV¿å!¢qPòƒ¿ëGóëZè•AGNbcu@×Ã")´PowerLawPKS 0042-373?ïþ]CÁ»?(ˆ€îÿã?.Ê)šAD?(ˆ€îÿã?ïУ¦/K"?³Ÿ'h?w®,ϝè?³Ÿ'h?ï´~5KL–?{ëÅMŒ?'àrº"T}?{ëÅMŒ?ïÿ´òý>ô6]LÖ-?ÿÁªÞ>ô6]LÖ-?ïÿ>Çïuø?ϋé¨?'YP‹Ã?ϋé¨?ïe£Jì¾?¢
ì	¥†'?"K–»Êš8?¢
ì	¥†'?ïœûuÞ?'.[ï}C?}6c¼ Û?'.[ï}C?ïýʪë?)Œ̱V?1¯ãWv?)Œ̱VAGN3FGL J0045.3+2126@^CÀh ÓÀD³° F\À8Ú0òçÉÀ;Dþ`Ï6?á!€:ÍÜA@WÛ÷âû?þbw¾þX
¿â'T6@·^¿áOC¢Ê£Z¿Òøx‹›ÃÚ¿ácuxۑ"AGNbll@¢<<j~ùÛPowerLawGB6 J0045+2127?ïý0rÂù?-õ!Û°xp?6|k|®Ý?-õ!Û°xp?ïÌKù[SÁ?‹ÕÁs•]?yÚM†«^?‹ÕÁs•]?ï܆Íi8?pi³¢*I?q¼™[­¼?pi³¢*I?ïµ =w¯º?d̳nÏ8?'—ð«[x?d̳nÏ8?ï÷Ù×æö?M¹û%ÖA¤?PLOæ6*È?M¹û%ÖA¤?ï
cÒs'?±#,õ&i>?ž³…±ß°?±#,õ&i>?ï¦PQ¯¨­?†¡ê'|ìD?†k됦8¶?†¡ê'|ìD?îž`Ðû/·?'IˆO¾[?¦òò๒?'IˆO¾[AGN3FGL J0045.7+1217@^/l?Ä;.ÀIG™¦5À9AvK¶·¸À;n T3]û?ÀŸ.—@ëáwÔ¢Ú?ÿ[@š$¿¹W)˜»ßP¿Þwa¢ÿ–E¿à%Ùºµ·Ì¿áͳiEá-AGNbll@ ðkC•PowerLawGB6 J0045+1217?ïý;µ–X?6ØH_(Ý?7Ž!qñ?6ØH_(Ý?ïϯØAÂe?Œ²ª€ª[õ?x(¾Òyç?Œ²ª€ª[õ?ïÏòþöÒ?vËb÷Áw?x{†€"— ?vËb÷Áw?ïã‡F–ù?Qïå /K?lçx¦+6³?Qïå /K?ïùKãÙ-Ù?G*6<.ä?JÐp‡~ž?G*6<.ä?ïAŒ?¬jZ¼º?—Îoã]u?¬jZ¼º?ï"g~qþ~?‹É«›~êú?Šæ q>Ѓ?‹É«›~êú?ï-R÷§IŽ?†°«,^ÅÃ?šU¡†j8?†°«,^ÅÃAGN3FGL J0046.7-8419@rñŒ¨À@gM@$³>À9Âw»ù?òÀ;¤gHäu`¿ÛÖ'/€‡@'ML @¡€mΐ¿æ"œã·0?¿æŽ8'm«¿ë!ghïؖ¿ïÿŒDÇZGAGNfsrq@x»`˜PowerLawPKS 0044-84?ïô"¡76?W"9"?Wº¾I3Þ?W"9"?ïÍ@Áªô?'-eÇb³?y@_¾Æí—?'-eÇb³?ï'3sAb˜?-ÇÒ|»?s#9ö-à?-ÇÒ|»?ïïJN
'˜?JÃv~Þê?`µ±ê~§?JÃv~Þê?ïí³>RÃi?hBÄïxd?bLÁڗnÿ?hBÄïxd?ï¹EÜX0?²^s$h?è×=•Â?²^s$h?îÚîGhA?™xڂ#"?¢_1ùî?™xڂ#"?î¾,¿.\?"é[]Oºž?¤-5Äè:?"é[]OºžAGN3FGL J0047.0+5658@^•[á¨&$À"›!
À8¹R¼ev|À;\ êƲ×?×
Õ*ŒF@=ijý¤Ü@ËC =͖¿åXûRWvñ¿â4Ä¿àR+•:m¿èvK-GXQAGNbll@'Qⶮ}VPowerLawGB6 J0047+5657?ïùºjŽX?E•¶k?IUÒ¸
c?E•¶k?ùhŒ0?"h)/l¥?ˆÝ¬¼+Ø?"h)/l¥?ïÜ,"ÜÁ7?u•Gy`?qé¶)¬¨"?u•Gy`?ﮔÄXñ?h/àzÞ&?"ZÎð¢ñ°?h/àzÞ&?ïâô#}Þ}?mÔ3ñC?mÜmƒÚù?mÔ3ñC?휮b8?»l"ÒQ	ø?³ŒñN?»l"ÒQ	ø?îћv«Ô?žm)Ï?¢æHŸ±)¼?žm)Ï?í±%§âæ?Ÿ"Ô~7?²vÒÁV?Ÿ"Ô~7AGN3FGL J0047.5-2516@X`ñ7ÀUüæ?Ïù¨À9yEi–œÀ;¶T¶"¥?À7Šïuq@54wž@ZVߊ¿Œ¿âd+Xs^œ¿åFÝA¿Þëqø´1¿æ+
:¥"OTHERsbg@'öœ(õPowerLawNGC 253?ïþï+ÇY?Ʀß~t?!
Bw™ö?Ʀß~t?ïÒÁi"P?‡É¨Éðöä?vŸ|4Ál3?‡É¨Éðöä?ïëS"Àç?f û
)Á?d¬{ʁé?f û
)Á?ïÞW‡·€?Wê n?pÔ<9†Ž?Wê n?ïþ¸è5Ö?+¾ö•\?/DsAf?+¾ö•\?ï!')C"ó?®ÑQbe~I?›ÏºÒt7¨?®ÑQbe~I?ïÎ{8/œP?°Ü¬•×?xÂcÚsh'?°Ü¬•×?ï
Š{9Ý?‰b8¦±ý`?ž®¿p˜Ä]?‰b8¦±ý`AGN3FGL J0047.9+5447@^›û'ÃÀ $y?ÜäÈÀ:<‹ÂAÀ;ªU‰ŸP"¿Ó"m|҅ì@.‹@š?õVtªL?îé£%o·Y¿ç²õ «†¬¿â?ñÙ
s?á0êíZr#AGNbcu@Õ,6E¡ÊÁPowerLaw1RXS J004754.5+544758?ïýÂÑÝ?A¾HHqs?7W'§²?A¾HHqs?﵍˜.‹?'žNˆnç?'½Ü—Œ£c?'žNˆnç?ï!Ñ9Õ?—&+ê'Ñ?›ÅØÅ\Á?—&+ê'Ñ?ïÿ–kÅS?šŠg;2‡?
eP¥}?šŠg;2‡?ï÷¬ŸZή?U.F` Íj?P¦Á\do?U.F` Íj?îk‡–‡?·L§ý2®?©G†¢'$
?·L§ý2®?ï|!Üý$6?6ôcÄí?{Ähò0?6ôcÄí?ïøËk"ã°?X¸•Rû?LÒR¤¢{Å?X¸•RûAGN3FGL J0048.0+3950@^Ž&áY.À7$_ZÙjÀ9ݏRîº]À;¥e5
ÿ¿øbf	aÀ@×)_õ³÷?þna«¿Þús&pà›¿àÇLÏLÀ¿àc¯1±Rô¿Ä30×ÁÐùAGNbll@«)ÖOv`PowerLawB3 0045+395?ïÿÛè?
×£ï3ÔÏ?¿M½öU?
×£ï3ÔÏ?ïÌ>-Ñä(?ŒÈÕÎ?yàé,[€?ŒÈÕÎ?ïðv%â¾?ccvä»é?_á}@Å?ccvä»é?ïÿüÅ8ü>²»*¡Ò">¹Õ€J†>²»*¡Ò"?ïÿ1RÕ²F?\ÆÌC7u?Õ Ÿ¥l8?\ÆÌC7u?ïGu¥Ò¾?«¶wǪ?—KDšG?«¶wǪ?ïÖöˆvËR?zÄz—Û?t"»¤ýï
?zÄz—Û?ïÿÒd«/>÷'ÈÿØK>ö͖mÉ"'>÷'ÈÿØKAGN3FGL J0048.0+2236@^z)à¤&ÀD!Ðß´0À9,ƒöš%±À;™!|QŠ6?îá¾y!ÿÚ@îþj(½¹@ª  žŠ¿Ût'冓>¿æ¥ãµ$B2¿ãíw3µ‡¿ë/EcškAGNfsrq@Œc·Ÿ©~PowerLawNVSS J004802+223525?ïýðu`O?'¡#*‡Åx?0|V諟m?'¡#*‡Åx?ïËi§}L?'Ù6$z??zrËõH?'Ù6$z??
ë{?[÷Å(Q?‹~
C')?[÷Å(Q?ïí&OA~?CAò™Î€Ä?bêÙ¬žùê?CAò™Î€Ä?ïþg
ópr?&V£×C–?)P,×mÿ?&V£×C–?ï †yÇ?³$­5æh?›ï>1?³$­5æh?îÀè+ç©6?˜ŽÑdm/1?£ñ}Dõ?˜ŽÑdm/1?ïφS>Á?f'Z0[;2?x<öÍq£^?f'Z0[;2AGN3FGL J0049.4-5401@rùm`ûHÀO6@-íyÀ:}2Ȫ(À<Çhß½j¿ÿGDAùI­@ry-hmþ@%µ\Í¿æLÝÏ\&пäcieŽ¿ßúÍì\Š¿Ö ='tËÉAGNbcu@›K½VlôPowerLawPMN J0049-5402?ïÿ+ÎSÏO?vaHˆ¬?†.4"ÊB?vaHˆ¬?ïÞcF1£Í?ƒ»MôT¦?pÎ\änii?ƒ»MôT¦?ïëžÁnU?QŠ._î`ô?da>°&:]?QŠ._î`ô?ïÿûóMa>º.Ö[Mõ>À1Á@žÉ>º.Ö[Mõ?ïÿWž¢lý?+wÀŠ¦-?*fdž?+wÀŠ¦-?ïBí
ñ"?¯8'†æ5??—¢^H¼…£?¯8'†æ5??ïè"ѳ¼[?i@Ã5/?gk.im¸?i@Ã5/?ïÿ©ÅzŒÓ?æ¶è:æ?Ž§É©Ü‹?æ¶è:æAGN3FGL J0049.4-4149@s[6†¥ÀRÓ@ÃÀ:–²gƹÀ<"ę¿Û;óv.Û`@­"óoMì@<zßð&¿æðÊ㓍¼¿êöÇvõֿʪ 1'%¿È9[ã¢ô"AGNbcu@¡€ûçl‹DPowerLaw1RXS J004939.9-415133?ïþ¸Ífz³?*q!È9Â7?$s'B2gà?*q!È9Â7?ïÙ֒KW?"_†JIá´?s¶ã,èÈ?"_†JIá´?ïÐ>«P?!?vfLKnN£?wàª:SËs?vfLKnN£?ïþçCàC?X®k'?/‹Z¡#Ê?X®k'?ïþÁst¹2?:	yæ÷Ìz?#èË2$^¿?:	yæ÷Ìz?ï2Iû"?²…¨™¦TŸ?™¶Ì=,q¨?²…¨™¦TŸ?ï¹U¹´±?…Õ­ä,Ïg?¿*‰«¹Ñ?…Õ­ä,Ïg?ïîÏ=ëH
?Xrbš•GC?a0Áõ‹"?Xrbš•GCAGN3FGL J0049.7+0237@^…п "`ÀNJÀ²¤À9h"t¼À;°â`²È?'ãY,@è(©c@óËßgD¿ã,ï!¿äºjþÚ¿Ý0r‡B:¿è<IiÖ]oAGNbll@òF?PowerLawPKS 0047+023?ïÿ¾-;'?>ùŽV?t¡<ÅÎ>ùŽV?ïÖjoàb¬?‹³ã‹™ëh?tÊÇð2BI?‹³ã‹™ëh?ïîliW(þ?hî[Ãð7:?a"–Âô	¾?hî[Ãð7:?ï÷
»sx?7Œåóá›?Qëâñ/®?7Œåóá›?ïÿÇöÏ)É>ø[Ôúø>ü™¼às×>ø[Ôúø?ïf®@<(?¦Êò''¼?">
/au?¦Êò''¼?ïçûÅfY¯?p/ô'2>?h:'gA;?p/ô'2>?ïÌ]åtŸ ?hÕ&—?yÑ
@à»Ü?hÕ&—AGN3FGL J0049.8-5737@rõœýç!ÀMÀR@>´qÀ9ҝë7òÀ;ØÌð;8¿½Q‡Ðw@‡ùZ"z@²'€Ê÷¿èà{ô-å¿åòˆá±O¿åîôŒÚD¿Ò®D$ТAGNfsrq@Qg8}¿PowerLawPKS 0047-579?ïþ`47?)`Bi¥…?)üº§ ÷?)`Bi¥…?ïÛ2"ý??…	­ö™?rfµÁ@p>?…	­ö™?ïÏþ³#ÙN?fÿs4ëC?x¦tòï?fÿs4ëC?ïùQëE?56€L\?K'¸¤h?56€L\?ïû–zïú?J¦Ô›M*·?A¦X~˜?J¦Ô›M*·?ïNÐ>‹é?©®¼?–%ø)uXí?©®¼?ïZ­Ôm?‹™\¨ó?¼á®lv?‹™\¨ó?àŎP?{ªaý©?ˆÇÕ{£ä?{ªaý©AGN3FGL J0050.0-4458@rû¯_Ô{îÀR	â H¤À:NÈ>Ȓ«À<Üq…~Z¿ãP€èa—Ž@è«,¾úÒ@9Ÿ…@ò¿ç³Zh‰à¿ààêZɜŽ¿ä*NãgîÒ¿ïÿ—w«];AGNbcu@…¯úxl"hPowerLawPMN J0049-4457?ïô'<Ÿ‡^?U"Ñ{ß$¸?Vû†hûDA?U"Ñ{ß$¸?ïÓ5ƒçÍü?
"ÉúI-?ve=ú;	á?
"ÉúI-?ïńÍË?þi,2p½?œGOs%~¤?þi,2p½?ïû
*q)?/Ì#"qJ—?AËÊÿë"?/Ì#"qJ—?ïøcéUæß?Q˜u"[–?NpZÈGKA?Q˜u"[–?ï<F‡£ÍÐ?±(ŽU²±?˜w/Kô?±(ŽU²±?îÂj=‹{Ê?šð½ÃRÒ?£Ù\)Ûøb?šð½ÃRÒ?ïÇÛݔŠ?p»ÍY8MH?|F¿
?p»ÍY8MHAGN3FGL J0050.4-0449@^"¤as¸_ÀPìû_ò®ßÀ9ž±ý=­àÀ;§Ôî~:¿Ön>ڎà@'
ǾÅù@™\ÀJ]q¿á—:f®4Ü¿æ"Q¦ùT¿ä@Î>p´¿í"Ó_Å|AGNfsrq@‰¿-ÿ'+¿PowerLawPKS 0047-051?ïõ1ð½í·?UžÏŒeá?Uœÿց°?UžÏŒeá?ïÔ£0–î?Š3¦#)u¦?u®xp£"ì?Š3¦#)u¦?ï"Àgm2?…¬®ý·ƒî?ŽÏæD³‡X?…¬®ý·ƒî?ïóÛ3G´?DԙÏÆq?XIçØ©h[?DԙÏÆq?ï÷å¥id%?Qü©\ýÖ^?P4µ4]KÄ?Qü©\ýÖ^?ï2Ÿ äs?®ØÃJùë—?™¬è˜ú?®ØÃJùë—?ï+¯¹@¨è?•rÔÚH?šŠÑ«?•rÔÚH?ïu'î(ßj?ÂÇG<?'O¢9,DÍ?ÂÇG<AGN3FGL J0050.6-0929@^•-û¹ÀRÄ`Á
À7ï;M;À;
;…è?ÌÚ#ޒ®)@ø‡©'ö@¾ž²gÇ¿Ýè%Õ#¿âËÿóγ¿áíT<ÿK¿ádiÛ±ÖAGNBLL@ø"µÜÆ?PowerLawPKS 0048-09?ïÿÏ	¬ÀØ>ñ‹´°[ü>ø{Dª¬>ñ‹´°[ü?ïÙõTUlÄ?ƒXz›Ž?sUâX!ò?ƒXz›Ž?ïè+‹Û&=?n(º.õ—?gÔtCRÄ?n(º.õ—?ïÿx9çF:?å·7']M?ø¼ìR½?å·7']M?ïÿ¹–²¿>ÿ™<Ë\?šnÍè.q>ÿ™<Ë\?ïP,‹¬ÏŠ?«ìk|"$?•únˆ®@Ä?«ìk|"$?ïæTmj'™?s6ÞþŠ ?i«'€Ð¾Ø?s6ÞþŠ ?ïþ£B ;? %
{†JL?%Ëޞã? %
{†JLAGN3FGL J0051.0-0649@^ª`4óþÀQlÆøÀ9'Þ³íÀ;€X‹Ž>?öÛ)üþ˜Í@]‰~noõ?þôwÉe9@¿ÛÐ\ùпäñÕøO¿åwåiÑ«¿ìh­ø AGNfsrq@†§€uMLogParabolaPKS 0048-071?ïÇß'ËԈ?|d{훫@?|l
8"?|d{훫@?ïȌf*Vk?ŒžU4¹µ?{¹ÌæV¤?ŒžU4¹µ?ëÆZ¿¿?§ù:`pz‰?À瞕‹?§ù:`pz‰?ï»,˜Ü§®?cw‡Ê†ðÎ?4Ù¾/J¥?cw‡Ê†ðÎ?ïˆƹ7o?‰ÚÇGïS?þÎCó´h?‰ÚÇGïS?îù')Ä°°?³pÒ
¾? fífHª?³pÒ
¾?ê…gô֊?®ãÕXà·?Åêc",¥Ù?®ãÕXà·?ïe
*r¼­?'éúêèC?"^º©d_?'éúêèCAGN3FGL J0051.2-6241@rïj_"ÊÕÀK8X R…ßÀ8Ô¢ŠÙã6À;ÝS¨?ãiËÙìÙ@SBïòÌ?úœF__áè¿å.w†Á¿Ó3h7Kñ›¿Ì{fLTU¿Ó)ÈÐ,ÂpAGNbcu@®{6ý!ÿ.PowerLaw1RXS J005117.7-624154?ïô½Îq?P75)?V"c™°ÕE?P75)?ïÔDGO`?'sÁsHf<?uÝÜGö°?'sÁsHf<?ï¬êH«ÿ?Õ´žc?"ÅmÇ~F?Õ´žc?ïÀ<ËãBÛ?b´·ÍNÃ?ášB"?b´·ÍNÃ?ïۇÒ©?r8…7£å?r<8|µ"Ž?r8…7£å?îØFE½,#?²–»Naê?¢{›¢uoË?²–»Naê?ïJ1$mÑ?'ڐ'†kD?–¹ÛrEÜr?'ڐ'†kD?î×ހÔPÐ?‹èä›ÐŸx?¢'ïKW
?‹èä›ÐŸxAGN3FGL J0054.8-2455@aÐØ`fÀUêeà.©aÀ9G±CÝ¥À;Ph¯ìÂ6?ÛgÓ`¸@ÕÄÉH3?ürå?µL¨?íš®t>Ž¿Ýb=ºd¿Ó<ؘ£Ù¿àtuȯAGNbll@¦¸Ý/ PowerLawFRBA J0054-2455?ïúõc¼4q?>|Eá`N?D*qyÕPB?>|Eá`N?ïЦ<±?‡êLuµŸñ?w¬ôˆ/;e?‡êLuµŸñ?ïŨ
 —æ?z™~A?}+ú½r}%?z™~A?ï½`7(
?fq¦¯ƒp?€§ò:V%n?fq¦¯ƒp?ïò\}Ñ´`?W-£âªÒú?[G6¡?W-£âªÒú?îþKJT9?±ɁùÝ? KbŽqq?±ɁùÝ?ï™Ñ€÷È_?‡J8ƒW
?‰‹ŸÅ}",?‡J8ƒW
?ïê{æš?ˆ'ˬ㹨?žâ¼é£ôÇ?ˆ'ˬ㹨AGN3FGL J0055.2-1213@_ ©?)
»ÀRÄÿ¿ÓÀÀ:xHG—nFÀ;ö
>¬ãù¿àÓ|¶¬F@ìŸf7A‹@,€0¥¿á †N
!¿çÖ´ñӆ>¿äü—öV^¿ÛºßáÛíAGNbcu@%È÷QPowerLawTXS 0052-125?ïÿ¥hɆá?	1"[²še?¥Ù`M¨l?	1"[²še?ïÚJ¹.+Ú?‡bË&Y†?rÚ£€Gjý?‡bË&Y†?ïì?d«˜?\—'_¦"æ?cÀ›Z€+?\—'_¦"æ?ïÿj"i L?ÚõNގµ?­"Ôk)Â?ÚõNގµ?ïÿ")'Ò?:0ã<Tq?
õœ'œd?:0ã<Tq?ï_(›™gß?¥<žnz
?"ì'ún?¥<žnz
?ïÌDÕÙ!*?€(ª7ÞS?yݕ's?€(ª7ÞS?ïú½ðTÖ
?<y(AúO?E>é­´ˆ?<y(AúOAGN3FGL J0056.3-2116@`½ë¿×ÀU
€!"À9•ÄÿxñƒÀ;vÖ
c0Q?àÙo@`Ö#7½‡?üí~@!Ù? ïÃ
J/¿ÒºJ†-x¿ÛÅð Í§¿Ù×RH'ÖAGNbll@¦PñA [ÀPowerLawPMN J0056-2117?ïþZpäĐ?#4ÁžKð‰?*Xïs'ä?#4ÁžKð‰?ïÜ&d׍?})ViYçþ?qìÎ
Á¥S?})ViYçþ?ï׿ܛÄ9?rn¤ÁŸ€ç?t ½ÌŸ?rn¤ÁŸ€ç?ïãÕÂ6=?Lã‹Ìúfb?lì*hdêz?Lã‹Ìúfb?ïû²Þ
?;ÛÄ2èq?A4…íø¢—?;ÛÄ2èq?ï0+›((Ø?¯Ûígç—?™úŒ—‹I
?¯Ûígç—?ï³ç]Pœ?ƒƒÀ¢¯~?ƒ?؅¯+?ƒƒÀ¢¯~?ïˆÓ_Ÿ?uBS´Ío'?ÿ>Õvì%?uBS´Ío'AGN3FGL J0056.3-0935@_½^	ÀRSÍ$áÀ9ÁÕùµcÀ;|Fûg¿³Õ¥½@8@7s'À?ü¤À Áìt?ìÏ96Ç+¿Þ$ÖxQ¿Úç0‹c ¿Â^P»HAGNbll@¯'j=p£×PowerLawTXS 0053-098?ïêÕ	öè™?šíL¥ô;"?e*õ÷9o$?šíL¥ô;"?ïßfÞ9r?|à¢ù$Ä?pLñ76ä?|à¢ù$Ä?ïߐ,n¯?p¼Iÿä@?p7鶎a?p¼Iÿä@?ïþeá—?xQ¾f'?/‰ oõE/?xQ¾f'?ïþç}Ž\?(åšÖS)-?.1‹êh|?(åšÖS)-?ïj"³MAI?¦ÿh6Nä?'­i'0lï?¦ÿh6Nä?ハÇÄ¥6?'â¡!ܟW?€]N	WR†?'â¡!ܟW?ï÷—B?FcõoéÍ%?QÚÑÇÜ@¿?FcõoéÍ%AGN3FGL J0057.9-0542@_ÖNaŒâÒÀQ!ŽèӔÀ:43#Bû'À;¶Ï†»p"¿ïzI²‡@,
{®÷û@R²à£¿à¼‰ô
(x¿æÒå•Ò¿å_ï˟J¿æ¤´ïz;AGNfsrq@''?b¶®}PowerLawPKS 0055-059?ïþÔxV—«?(V¯ü‹
S?"¸vôUy¶?(V¯ü‹
S?ïÔ²µRu?®\ñ³ç?u¦¥dÉv?®\ñ³ç?גּ¿º@?Ð…ó+Q¯?"ÓzÏà?Ð…ó+Q¯?ïþ½H({?Éâûзx?$+€3Y…@?Éâûзx?ïø:x:¾?Z)ǗãE?OäE×?Z)ǗãE?ï¶fg?µýØ2C?	<î©?µýØ2C?î@"N²W?§ÈɯwW?«÷»Xó?§ÈɯwW?ïéÔՄ×@?_m&!9z?f+*šÅ(?_m&!9zAGN3FGL J0058.0-3233@r	€bïÀU¿ÖDEÀ9C'5ÏÆÀ;€Æ'—¾?ï+I˜¶€ì@¢Ž>F·Ÿ@w~?ËòÝ¿Ü«#ñ2¿ÞšMìût¿ãX^v‹€/¿âm+©û~AGNbll@"!Tã¼Ó[PowerLawPKS 0055-328?ïøÍ6)1Ó?F\Øe"† ?LË(6'÷×?F\Øe"† ?<r!0?—¦Vﺈ^?Ú0ñ6$?—¦Vﺈ^?ïËG9Õ?xZÑØÞQ§?z\sì´eL?xZÑØÞQ§?î/=-ı?‹ˆZ	¿O?­- NÈô?‹ˆZ	¿O?ïõzÛ4æß?SÞ¦-ñ"Í?U
Iÿ²Ò?SÞ¦-ñ"Í?ë†!·úr?é;˜\'¸?Áæy :?é;˜\'¸?îâJé:õ'?™ŠZþÆP?¡ÛQoÀIŠ?™ŠZþÆP?æYµ±…Ò?µ«¾;7Ú?ÒåL"œô\?µ«¾;7ÚAGN3FGL J0058.3+3315@_%þKZÀ=•2¯ÈÀ9ή"i›À;й!õN?ÑÞüûÛO@ç0+kéˆ@B"@Îé¿æTgê䩧¿â.ñ°¿æ[š6nô¿íËLŽ'JAGNfsrq@ˆ­À6ãPowerLawMG3 J005830+3311?ïïÊyû?\"#144Î?`5…Ä_ËÚ?\"#144Î?ïÍIº¼²?‰æ
&qK?y["¹c?‰æ
&qK?ï
ìWè°?eÆEƒž¯?žNz*Sì?eÆEƒž¯?ïìAº¾
?F/ϦýªJ?c¾E†®¹?F/ϦýªJ?ïÕ	‹ˆÎŠ?xéx¼ð¯Ø?u{:+›?xéx¼ð¯Ø?ï8¸ršÅ?§YýÙQn?˜èñµSMI?§YýÙQn?îÐwö?¡ò?")ˀ?¯'øŽÑ<?¡ò?")ˀ?ïwrw@Ô?}B…<ëšÐ?''ª8­ƒ?}B…<ëšÐAGN3FGL J0059.0-7242e@râR€jôkÀF5W¿ÚvÀ7îjCj¹À:ô‹…à_?í]ñg¶È@AT;9½@đ #a¿ÛÆ2x'É¿ä•×m9¿>¿ävôô3C#¿è"äÞ¼csOTHERGAL@"ÌAž0PPowerLawSMC?î],³^´
?°qWÂDï¯?ª-4Ë̍0?°qWÂDï¯?ç-Kú]?Í
Súí¶@?Ñ¥ÓhEó?Í
Súí¶@?ìTx¡Á3?¨|"g_óv?½\:ñ÷e?¨|"g_óv?ä+!S.G³?²å
J–!?ש½Y£p™?²å
J–!?ëODnÍp¿?ÁÄ­
ê¤N?ÂÂîDÊ=?ÁÄ­
ê¤N?ÔÙÃMРõ?҆	a¿ä?å"Y¯…?҆	a¿ä?åÏ;y,M?¸3©§ÑD?Ôa‰ñ
§f?¸3©§ÑD?¿áJ~ÔF?ªší–@Ö?ìÜÖ°%w?ªší–@ÖMIXED3FGL J0059.1-5701@rÍÆøÀN	T9À9~@¡°À;ÉS¿šµ?î°–7@¨•žÃû@îpnö¿ÞTíPo¿ç•>&þ¿ëH_TÉ¿ïÿåώY[AGNbcu@AE¸QìPowerLawPKS 0056-572?ïÁoAèhñ?Ÿvò3?H^îîÏÈ?Ÿvò3?í
ƒ=YL?º\,Ú1Aõ?·"æí3$?º\,Ú1Aõ?îÛÞՅO'?"3Ñh½Ù•?¢B¥Râ?"3Ñh½Ù•?èì1¼"?¥TH]´?ÌO9
½­Ë?¥TH]´?Î>¼Ô?ŸvàDy?\zŸžå?ŸvàDy?à쯃ï@ô?Ò÷åÄ{¬?Þ& ø!~?Ò÷åÄ{¬?ë£bø?°yÇ"|?ÁsïþwŒ ?°yÇ"|?ÍPN®~?±ÏÄHbÓ?è«ìX"|à?±ÏÄHbÓMIXED3FGL J0059.2-0152@_߂¡/ÀP+á .QÀ:k+D´À;½¦læ³(¿Ô·Qª0"q@ï9}$C?ûÍ[ d¹é¿Øµ{!‰g¿ë´kÏhç?»¹=ìÓ0¿Í²w°}þAGNbll@·éû¥ãSøPowerLaw1RXS J005916.3-015030?ïÿ™z‡R?Îu:îä?	¡\,n?t?Îu:îä?ïÙU»z{?"æà嬙[?sUw2öT?"æà嬙[?ïÚVûºK?qâ€nÌz»?rԂ-Ù5s?qâ€nÌz»?ïþóò;ØZ?kÜjÕ? ÀàIÑîô?kÜjÕ?ïÿn¤Â?bô&
Öv??Nùp\?bô&
Öv?ï%‰«©«N?³BoÀ$?›Nʊʖ3?³BoÀ$?ïÉnX£/E?|솹ÛJ?{HÓ¥yaÄ?|솹ÛJ?ïû؝²ÐD?</EÃ?@ˆº³7ó?</EÃAGN3FGL J0059.6+0003@_ÙØà†8ÀO_Ï¿ÆT
À:J'ÇÅ&À;ϸé?á÷÷ßA'@¢éCÐå5@ß&_3i¿ãÓÕ!&Ž¿æ5h¡Bõ¿çÀµQRzn¿ìŠðð~¿AGNfsrq@‰'9ÀëíúPowerLawPKS 0056-00?ïëV%Y3?"ë²s¸¼þ?d©ÚÎÿ‹?"ë²s¸¼þ?ï»k {Ð?^ÙŒv,?9åðÐ?^ÙŒv,?ïR"u¾2?‡xràû¶x?•­'F"‹Ð?‡xràû¶x?ï	"˜Ñm?zØ9…d×?žÍm¼Øc?zØ9…d×?ïê3lˆ-?eí
8ùÕÉ?eÌìhܪì?eí
8ùÕÉ?íݶ††¹º?µ$ %'kz?±K͂*?µ$ %'kz?îÎÐÐ<?˜gAÜÂ?£þj–±9?˜gAÜÂ?èB!÷\Ô~?­×ϳ|±¼?Î÷x"Œ®
?­×ϳ|±¼AGN3FGL J0100.2+0745@_°4?¢­?ÀK…à
—3À8«sp:$¿À;
{¬HÈÇ?óîCÍ_CÝ@«wènê?ü¾ÌßAC—¿ÂhÍÿ|Í[¿Ó¾Å4ts<¿Øw=N?(¿ÛþNuÀÒAGNbll@¤µmÅÖ8†PowerLawGB6 J0100+0745?ïþnQ[+9?*:ñ6X?)ìMf?*:ñ6X?ïÃjö˜ù?ˆVC;e?~J"¥Å
±?ˆVC;e?ï^Á;Ê?\}í1?j?">‡Ç€À?\}í1?j?ïS]§ïe?o¼I½gx?•"K¢Ûl?o¼I½gx?ïýå0pá?5ýÓ¯b?3Ø㎾?5ýÓ¯b?îÀàã&£?²3¸~6<?£þôaJÐ?²3¸~6<?ïÜÝ;â?˜ø™˜è¥¹?œDd_°Q²?˜ø™˜è¥¹?îNçg,à?'9ì9_Ù?«A‡Õd?'9ì9_ÙAGN3FGL J0101.0-6422@rÓ[ߏG0ÀJ\ŒSâÖÀ9õ[aO¦À;Ê~ÀÐ?H?þÃ	õ¢.@
~×ÌZ6@FÂ5D/…¿Õ€ÉÈ¥9¥¿Û'hÉþÅ¿çM‹È>H¿î+
Ö
áPSRPSR@Œ6sbb˧PLExpCutoffPSR J0101-6422?C«õËSB?Jú(¬H%?ïû>•¶?Jú(¬H%?Ã¾G|u?ϕôhȃ?ë<Ðn ã?ϕôhȃ?¹è3º#þ?¦³n@ ::?ìÂùŸh»€?¦³n@ ::?´>…»ó	?"·ÆÒÎÏ?íx/H]M?"·ÆÒÎÏ?Su(š¸?O§&‰Ê™b?ïöqE‰ïO?O§&‰Ê™b?µÆ@uäe?Æ"ËéÅMt?íG7þZI´?Æ"ËéÅMt?«).ïÎüÊ?¡XÐ_U/o?îMm3?¡XÐ_U/o?ƒW¹]àU?sŸ/8?ï²£àç®G?sŸ/8PSR3FGL J0102.3+4217@_Eð¡¾+IÀ4‰xmžiÀ9SDñ¡˜À;Â"³‰.è?éSGà¿Gÿ@š€Ê?Õ@ˆˆŸÌ8¨¿æÔŸÚrÊ¿èžr!c/®¿ë…܇n¸‰¿ïü-êì>úAGNfsrq@y›ºÜ	€²PowerLawGB6 J0102+4214?ïü¹ƒ2¾³?;¼n%pß?:3è€g? ?;¼n%pß?ï"8êŠÖf?"€nYðy?ŽñÅkÖv?"€nYðy?甆5Ié?rÐX}?…WrŸÞð?rÐX}?î© 'gÍð?²"i2Ö?¥mý†…?²"i2Ö?ïú2í,¥?P|ëon‡¦?G7ìî>Ó?P|ëon‡¦?í
A÷=±?¹ˆ†Wåž?·•ðDZ©Ã?¹ˆ†Wåž?ï!‡,–?ˆÃA&ɔõ?‹÷»æ?ˆÃA&ɔõ?æ£3y1Î?®¸íÿ˜?Ò¹õ™
œe?®¸íÿ˜AGN3FGL J0102.8+4840@_7ƒ]íñáÀ,Oö¿ž(À8ÏϚ¦ãÀ;MIðäÚ
?úÝÙìD@­AÂ<@œuhâÿã?‹þrى¿Û®Ó朂¿å‡)yù\¿ê-s>¢8`PSRPSR@'©Dg8PLExpCutoffPSR J0102+4839?ÌV¦þ›?Å4¤.jmÿ?èêV@\9?Å4¤.jmÿ?¿eÑýŠk?ÄATö7»?ìEÀ\.³?ÄATö7»?ä!Õ™êø?¶ÌhíJð?×¼UÖÌ*?¶ÌhíJð?ђ|…r×I?¢Ÿ]!õòV?ç6Á½F"[?¢Ÿ]!õòV?'Êtíº›ƒ?—³,?ï´Ö,X3Ú?—³,?¡'"¤;?¬¥Ôü ?î}¿|?¬¥Ôü ?ɪš¬ØÕ^?´À™ªäÚ0?é•YTÉÊ©?´À™ªäÚ0?§ª›÷!G?Œú)œô|p?î…V@©ho?Œú)œô|pMIXED3FGL J0102.8+5825@_B€®IÀ¨!ßβ*À7‹dBSbÀ:ú3ºA¯Î?ú‡Çßþù@;ºjŸ†@²,±¹Ëé¿ÝƬ_¢…"¿ãÔ"‰Sw¿åЭh>¾é¿æÙ¾«T‹AGNfsrq@€0‹'»0LogParabolaTXS 0059+581?ïûCÅ҇¢?GÊÍÇå#?Bðè&ñ¹?GÊÍÇå#?sÀ'^?­[ÌÄê*V?‹™£eÄr?­[ÌÄê*V?ïðrn\?–IdþÔ©?ñ«U8)?–IdþÔ©?ïþaBà?Ö#¾Cý*?)ïUpŸ¿?Ö#¾Cý*?ïê
ùêMw?pÓÎdJ¯?eõOkøH?pÓÎdJ¯?íõ£û
}?¿Mmq¢Î?°Rçݹš?¿Mmq¢Î?î‡ì,'j?›1U$¯Ñ?§=@œ?›1U$¯Ñ?ïþ­ßÄ¿?"ÝùYªQ?%"¤ ¬?"ÝùYªQAGN3FGL J0103.4+5336@_/0¾
í)À"mµ'm,À9š<Z#bÀ;•µav<¿õr`''èu@®µ©D²@Oë L'(¿à…Œ¿âõ¬¸}¿ßµë–³Ø'¿Ô=ڟ%þAGNbll@¤›²-VPowerLaw1RXS J010325.9+533721?ïþ+2ß?.B»öÌ?/¹M۞?.B»öÌ?ïɦ¼Ãþ?‰;ò­-¶w?{,¢¼èí?‰;ò­-¶w?ïßN*kŸœ?is`d:…?pXêçé›?is`d:…?ïÿÚþéª~>钝½>ò€†Ê!§ù>钝½?ïöó±Šsƒ?NˆfG²ô?Rœ…d‰ê?NˆfG²ô?îêbñ€¥?ªsÒS­"Ï?¡YÐèѕR?ªsÒS­"Ï?嘆õ'×?"Ô9ã•Í?…Ò"ûgN?"Ô9ã•Í?ïýT0¦2|?4TôŽÖìß?5^z9ýÑ?4TôŽÖìßAGN3FGL J0103.7+1323@_âx £
·ÀH¯8à^*À:-m\ú¬ÚÀ;ËVN?ì~fº–Œ@º"kì­?ÿ½'ÓY¿èGr°K¸?––á"–5È¿×Q\`uƒ¿è?iÔÉúAGNbcu@£/?;dZPowerLawNVSS J010345+132346?ïùL0žó?JLÕ®ÃE?JÏ>ŠüJ"?JLÕ®ÃE?ï˜ûÌ6g?‡íµÂÈ{ª?‰ÁáKA?‡íµÂÈ{ª?ïÁrü ø?{=ç?âg—?~F`CX?{=ç?âg—?îkh‡<?…7kÛ?©Iw…WH?…7kÛ?ïïjïÀ L?cIb½Ãÿ!?`•pÚw?cIb½Ãÿ!?í—Âk—J+?´Â(*>ãƒ?³Aì¢×»%?´Â(*>ãƒ?öEŒ?£mìÁ¯™R?§–@ÏÀ9?£mìÁ¯™R?é» L·Ò?­'FŽ&@S?É~Ïá ¹?­'FŽ&@SAGN3FGL J0105.1-2415@eZ`˜ÀUréÅ+À9jÑáÃôÀ;Üó…ô¡?뀾iW@@(4'@Ý砍©¡¿åË,AZ¿è'þO{¾<¿èåx.(Ì¿èΆ¢éE÷AGNfsrq@{£ì"h	ÕPowerLawPKS 0102-245?ïÿ7¥€$?ªFÜa?M@2 ?ªFÜa?ﻐ#p"à?"È®\ð?÷û?"È®\ð?ïÑ©ïŽSü?jô@­™?w+E4™»?jô@­™?ïù'{é?|PôX9Ïp?]@ÆñJî?|PôX9Ïp?ïÿƒÓ£o?ñ¶SV@K?¯´¤†?ñ¶SV@K?îs¼)*`?¶døOÔ?¯¸Ä;µŒ	?¶døOÔ?籠cÒbc?ƒ·f¾bí.?†žç×>?ƒ·f¾bí.?ê2(R?®S±ì—ZŠ?Ǔ7_'·¨?®S±ì—ZŠAGN3FGL J0105.3+3928@_va€M˜9À7R_>SùÀ9î㾀ٯÀ;Þ
,8m/?Ó,×(ñ:ë@¼e$@›|ßy¢®¿æO¶{ý|m¿ç´2°	%K¿Úµ†HÂb¿ì@÷33™AGNbll@'‹àÞ҉PowerLawGB6 J0105+3928?ïüB®{S?@ýW_9_ž??è·Á´?@ýW_9_ž?ïÇ"-CÛ?‰nôF¼¼"?|~¶h®&†?‰nôF¼¼"?嗀Çö› ?Ëþær?…ÜŽ	8P
?Ëþær?ïÈUÔÈĪ?^6Á̀Y&?{Õ†Pé?^6Á̀Y&?ïúietN?HCâ·³P{?FZj¾Ñ"`?HCâ·³P{?îâ[W¤?®ÈÁŽûçà?¡ÚHÍñõ?®ÈÁŽûçà?ïn6–úö?'IÒ\?'9-8ÁiL?'IÒ\?îŽ=Îþ¼o?•YðmX '?§#8R
?•YðmX 'AGN3FGL J0106.5+4855@_^́'²ÌÀ+¾øßzN{À8®=Ç᫁À;Sà0Vßá@Úi=DY@
֛©"8‡?÷T™"öÊL?èÃQ¿Ù(…ÈßàÙ¿áêe¿ïá¼hÚ·PSRPSR@—…ݗö+PLExpCutoffLAT PSR J0106+4855?CuR4ƒ†º?Kß¹	½s?ïû"«P¦6?Kß¹	½s?§T:Þ°÷p?»"kòŽÊ«?QÝöÉ?»"kòŽÊ«?§$öP÷
Û?›[ûìY‹á?šðR?›[ûìY‹á?Œùs®Tdý?rZš¨$ÞD?ïŒ1s?rZš¨$ÞD?W4s²¯?bԈ߶T(?ïôeÆ6
a?bԈ߶T(?"{ 'å¨ï?®¿*'ø|Û?ï\"û$‰?®¿*'ø|Û?'m¥06å«?‹™Ö~?ïl'Ö9£?‹™Ö~?d‡3Ûº©q?U2+iAåa?ïëẋ?U2+iAåaPSR3FGL J0107.0-1208@a.T2TçÀR¤• Õ`À:l,µÿ+À;äkŽÄS'¿¢—z\Få³@åN`¶#=@qŸš´¿æK£ê«Z¿à>'$e™¿ÝVÎ:WŒ¿ê±K}"÷AGNbcu@šT,<žíPowerLawPMN J0107-1211?ïðÄðy>?WÐu¯ÎC?^v€ö¢ñ?WÐu¯ÎC?ïÄʋe4ž?'î¥L›³&?}šºOutÓ?'î¥L›³&?ï4ô76?&›"(h?™ayY???&›"(h?ï®ù¸W?k·¶ìäæ?"AºˆÈ(2?k·¶ìäæ?ïؗiFHA?tˆŠSY²?s´KQÝZ?tˆŠSY²?î®ß
ìýš?²O	\où?¥"çôa?²O	\où?îU"_#T? vÅùÜÀÚ?ª­Ú…˜Ä? vÅùÜÀÚ?ì¾éÉ"?§ä"Þ†Ã?º±·?^?§ä"Þ†ÃAGN3FGL J0108.5-0035@`Ž2ßP]ÀO"!ÀD(NÀ:_-p{"À;ÍaÐÕp	?ç*Î$20Ì@$È´º1@&H «L¿à3×m5¿âÆïD4Ò	¿êÃPċ¿ïÿLˆ¼ AGNfsrq@T"Ðå`BPowerLawPKS 0105-008?ï¬ÉÐÕ+Q?'Ër'em?"͋ʵ+­?'Ër'em?îÚ{ÊâÍü?¥·\¼Þ1?¢XCPR??¥·\¼Þ1?î-3­Šý?—(Š¸«,¿?­,Å'^`*?—(Š¸«,¿?ëÞ@ûGßh?š"យrR?À†üà'a?š"យrR?î ö^…`?¯˜	 ´™?¯íð›Ïwú?¯˜	 ´™?æd]¡Š˜?Í£7–Þíû?Ó7D¼êÎã?Í£7–Þíû?ë´µ¡.†?°Þ^ˆ‹$B?ý-){Eé?°Þ^ˆ‹$B?ÖP€V㢸?³r" •(?ä׿Ԏ.¤?³r" •(MIXED3FGL J0108.7+0134@`{Ãá`xÀN	@¢CÀ7yÚh–ÂOÀ;Ù}µ7…?øn$Ù(OÕ@kä)µ°ü@Ÿå]½Jy¿â ÞÀŒš¿æ¶­ôøîq¿åe³™ÜÚ¿ê+\üŸBAGNfsrq@v	W>«6zLogParabola4C +01.02?ïõ磻~?UÇÁ蝮Á?T1ücR´¨?UÇÁ蝮Á?ïÆuhÍ?"ŒjQÅ?|öōIq?"ŒjQÅ?îü
]ãT?•J÷÷¨*? ?Z òcÁ?•J÷÷¨*?ïá"Žº?UHÜÅïµ?n€Ýâao?UHÜÅïµ?ïîˆÓgŠm?_
å'TV?aw,̯£?_
å'TV?ï7zŽ¢«Í?°DUô˜¶?™®0ÑðR?°DUô˜¶?ïÍfŽ?–ûߔ7 y?œ'ŽS.??–ûߔ7 y?ïÎX¨7ê?m';3=?xÓ¬1ž¨?m';3=AGN3FGL J0109.1+1816@`çßã*ÀF3=?üoRÀ9ÌjNRsjÀ;¸a†,ÕK¿â@2,…Ú@
§Ü"@k@Q–ߪõâ¿âÇ6cݿׯÛ[A*~¿âðÄQOû¿ÓÔèÍçÝ}AGNbll@¢HtêJŒPowerLawMG1 J010908+1816?ïþ‹3­à?'%ˆçµŒø?'LÆ~"Á?'%ˆçµŒø?ïÎڕQ$O?çTw ~î?x'µXÍ°§?çTw ~î?ïày½[?Â?mtÎâb?o†B{"î'?mtÎâb?ïý ' º?+!Y?ã×Ê?6ûﴛ˰?+!Y?ã×Ê?ïýK¸:Cž?/SIå²³%?5¢<&êáÑ?/SIå²³%?ï(À€¹"÷?µ¦³!nÔc?šçïç#Ó(?µ¦³!nÔc?ïÆ1âPB?~ÇW®™Ü7?|úgø§.?~ÇW®™Ü7?ïÔÔûáI?pcêÁÆß?už5rA'Ë?pcêÁÆßAGN3FGL J0109.8+6132@_H?Ffí¿óååÀ
̜À7³Ä UàÝÀ;TáÙ¤?ûÊÉĕF@µ|Ï'@'X³ö<2¿ãáÕRàÖ"¿ç?ÄEa*Š¿ëö•¿è¯ürŠi®AGNfsrq@tFÜ]cˆLogParabolaTXS 0106+612?ïÖ·P}Š´?®'ír¨¡Ç?t¤W´,"	?®'ír¨¡Ç?ï¶-¡×^T?'8'Ⱦ?'t—Š(k?'8'Ⱦ?î{'+ú?.šƒ_¬Ÿ?¨M=Êù©?.šƒ_¬Ÿ?ïú\!5|0?2Œx¶Ÿ'?F{")•Y?2Œx¶Ÿ'?ïÄ×ü3uV?'œ	¨{"?}"ȸ±.?'œ	¨{"?íw"oÛI?Ãñò;!û?´F쀷Ä?Ãñò;!û?îù5'æ?¢ž¬#Æ?®l¤bP?¢ž¬#Æ?ïøŸþ¯ë7?HG™ž?M€µl9z?HG™žAGN3FGL J0109.9-4020@qÿ4?¢­?ÀS¿ä†þÀ:]Y#‡Ä…À;ÇOr.Å¿ÿô
]ᇚ@
~	æ]Â~?û£l`üD4¿îë]£–"ú?ï¾âá-¤J¿æÏÊ|ª9i¿ÉX­*ÅüNAGNbll@³"uPowerLawRBS 0158?ïü²d…u?6>éô6ß?:lÜàL<"?6>éô6ß?ïÝ"èn?‡‹ÙẔ?qq¶üHÍ?‡‹ÙẔ?者Îca
?€à¬`m>?…™YiM­?€à¬`m>?ïÿù¡…å÷>Ȇ®n[ñ>Éy^èH+Ñ>Ȇ®n[ñ?ïùôI'CÖ?DRb'Áw?H.ÚÌˈ•?DRb'Áw?ïo]]©(ƒ?¢ Ã%ü`[?'TCû·¯?¢ Ã%ü`[?ï{Ù6+yð?‡Õn·Ó?"Ù5iX?‡Õn·Ó?ïÿ=C=¨"?!ø—éÃE©?W™¹"¶?!ø—éÃE©AGN3FGL J0110.2+6806@_,‰a=1º@;N¿«§
À8´¿%DÀ;´öí1Ç¿ñÒف;)@Æp÷cú?ÿڑÿFq©¿Þª¯ iú¿âq«h#*¿ßíž
¿Öì,39¾=AGNbll@¨¬øüPHPowerLaw4C +67.04?ïôÀ(ς	?YŽ*üí?V­âŠNý?YŽ*üí?ïÀ±Ö§A"?'|ñ¥ñ­?§'·#?'|ñ¥ñ­?ïqÆNX}›?‹ê)t°'?'Ç66¨¬?‹ê)t°'?ïþZ¥É? ı)W|?*U¥ýsœ+? ı)W|?ïÛ;Tk_?kå£Ýç?rb@oçX'?kå£Ýç?îÇö[2øó?³,œ ◝?£€šQóÉ?³,œ ◝?ï2ÏR¹
x?'ÂWRøŒ?™¦ª–~ø?'ÂWRøŒ?ïØ
±Åñx?r
ܼ¦³?sú§4dœ?r
ܼ¦³AGN3FGL J0110.9-1254@a¶êá‹ÀRÄqýÌIÀ:pµÈ¤I À;Ó	¹½&¿ìÒÏbJÅC@ȍ¸dàÕ?þÍÉ¿|,K?Ú#pqpõO¿ÚÁÜÚ$¿ê30ïꑷ?ÊY1y´™AGNbll@ª_GE8ï5PowerLaw1RXS J011050.0-125455?ïí%òՍ?;Œ'‹´?bÚCºY?;Œ'‹´?ïސè-?…B‰¯Èƒ?p·üb	u?…B‰¯Èƒ?ï<ë CÏ?^¶4S?˜bžc`€&?^¶4S?ïÿ¼öëÚ.>ûåÏ]?Â<E'Q>ûåÏ]?ïíþ"Ci6?do:2vå?blÎtÁ˜?do:2vå?ï:_¨ø?°Õ
væC?˜¼´Jàñ?°Õ
væC?î;Zb]S?ŸÎú 3G?¬OJXþCÉ?ŸÎú 3G?ïø½)Õ?S»>CUiè?M¨$Uێ?S»>CUièAGN3FGL J0111.5+0535@`ƒ'ßüTzÀLvÆÀCQŽÀ:"#bۗkÀ;áž*øÒ¿Ï@h¡DB@»»+9¿"?þ«®>Â2•?츝ü]fÁ¿ÙqÃÇj=¿ËåòFÈ«¿â(4æezAGNbll@­Š#S÷ÎÙPowerLaw1RXS J011130.5+053612?ïÿS)?5í?å)í8ñ?šÝ<Fiò?å)í8ñ?ï׀¸Á_?'B¼Ÿ[?t?£¥R\´?'B¼Ÿ[?ïáÖ'ª?eÎóákAÑ?n)úÀrÝ?eÎóákAÑ?ïû±|9av?(ÅÁ]£Ò¥?A:FÒ:ã?(ÅÁ]£Ò¥?ïþÒ|uW¬?$
l©ùüI?"Ø8‰ˆþ5?$
l©ùüI?ï;–ýïÜ?¯²*Ā¡F?˜ ;>,|?¯²*Ā¡F?ïØBI¯)+?tŠÍñáir?sÞÛD˜6?tŠÍñáir?ïîlÇÔj{?S]Œ™r)®?a"8IÒã?S]Œ™r)®AGN3FGL J0112.1+2245@`$›«–òÀCîŸóOîÀ7FëÝ3L^À:£!
;Ã%?ø>§UCÿ3@Å~öU1?ýøã
Hٿ؜t/ó¿àäJ\Å}οáC€»Û¿ã´¼~å§ÿAGNBLL@ƒ^iᰉ LogParabolaS2 0109+22?ïþlëCc
?*õf8£?)1O­÷¸?*õf8£?ïʋ'2Rk?'ÿ~³‹É?zº>ðu²U?'ÿ~³‹É?ï]"4‹ß?'‹'55Ü?"M™kƒÂ?'‹'55Ü?ïïžþÄ©?G,Æçhô?`ag~'o?G,Æçhô?ïû+y¢Ðœ?I€ü'¬ÁÅ?CRd(Æ?I€ü'¬ÁÅ?ï)QàóÊ?²gⓥ½(?šÕÄ`¾°?²gⓥ½(?ïÕi9»Ÿ?˜[ˆ%£´˜?œRÑéT3?˜[ˆ%£´˜?ïë'ü`þ?Zà=r\t?dØðÝ#bU?Zà=r\tAGN3FGL J0112.8+3207@`)?)
»À>†§ ÃY‡À7ùpQ¡³DÀ;]*Ãøèµ?ç Ü ›×@räOOt@æšà@œþ¿ã|Tò+¿å{{°iX£¿æŽ;@Œ¦Ü¿å±ÿaýÿAGNfsrq@€ÿ¸QìPowerLaw4C +31.03?ïÿ˜¨@5?¼Ï9ƒ?	ÕïÅââ0?¼Ï9ƒ?ïÔ)÷0‰Ç?‡²!§yê?uëSÍ`´?‡²!§yê?ï×'sé?s5™!t"ø?t|¶¶í0Õ?s5™!t"ø?ïÿ¾m͇>ï;AÒë
?d°….Õ >ï;AÒë
?ïÿ%îÜ·?BlàkñÔ?B7_¼'L?BlàkñÔ?ïRøé?ª23Þ¼¤?•½`é¼×?ª23Þ¼¤?ïxŒOvk?‹ßYO#?$?îvIÈ­?‹ßYO#?$?ïÿ"BË4O?êºÖc~f?
ïV	G-'?êºÖc~fAGN3FGL J0113.0-3554@qJ@WÀTLŸëÃ2À: W À<¾ne8i¿êøü^=@´½uÁÎ@ÈŠ>ˆ¿äGÃ*.C¿äódfº|Ç¿ïv­×û:Z?åeä J…,AGNfsrq@ƒ¬DÑ¢PowerLawPMN J0113-3551?ïÿÛ¦ôõ>ødáºW·>ò,zë²Ãî>ødáºW·?ïÑß+§¬?'¤€"¾WL?wŠx}¹?'¤€"¾WL?ï¹!`f¶Ý?±Ãq°M?·§Ú£œÌ?±Ãq°M?ïÿý)¨1>·'²è·¹ó>¶¸p¦ñ‰ò>·'²è·¹ó?ïÿÁò†ÎC?nñ@x>ÿÒ"BcŠ?nñ@x?ïN^¼ñ.ù?±ÚÒxÔ?–4(^j"Þ?±ÚÒxÔ?ï˜Äâ?B?‡å(«sJu?‰ÎÇs¨‹}?‡å(«sJu?ïÿ»ÊF	Ð?
ñÀîCÈ6?
dJÝí'?
ñÀîCÈ6AGN3FGL J0113.4+4948@_¥>¢ŒÀ)Í*Ž:ÁÀ9I݂&¶MÀ;ŒÚF2y?–ªnxåŒ:@æì·£ÅÂ@dŽÀ!ß¿ã¦oÓ¢~ð¿æeí;›ü9¿ââëYͿ൮#O¡AGNfsrq@'Š"'@·€PowerLawS4 0110+49?ïü‡^í¯?E7£‰@€þ?;Å
©ÞL?E7£‰@€þ?ï¯î¬_]Í?"˜Qx¡/?"TèØxª?"˜Qx¡/?ï̆ Á	?xJN[.†?y¼û¨ÀC¡?xJN[.†?ïÝ°yçá?VÕxz·—Œ?q'Ãf
Op?VÕxz·—Œ?ïëþb4í6?fm<ƾ@œ?dÓQٌ?fm<ƾ@œ?î&qòò·~?¶,qÍJ?­˜àÍdì!?¶,qÍJ?ï2Ñ#n?–Ѭ,.·B?™¿%ØZU?–Ѭ,.·B?îbj5}æ5?—Ç$hÖ]c?©Ù\¨!œ³?—Ç$hÖ]cAGN3FGL J0114.8+1326@`tÿ´€¦ÀH…>ÏuÀ8õ¾smµæÀ;oU"‡"¿ü¸0ÆFuÛ@wFwÉM@žL?ž¦t¿×dÄ9Lʿ怲u¾æ¿Ýe­›{"l¿ØtiD£YGAGNbll@–~¢Ðå`BPowerLawGB6 J0114+1325?ïÿà0½ô(>æjTëLû>ïÏQ‰Ds>æjTëLû?ïÎËy){h?Ÿ¥ÖÎ?xšCPuX?Ÿ¥ÖÎ?ïî=ƒ¡¾?\¾"]?*H?aó»—t?\¾"]?*H?ïÿþq¤Ké>©H]Œi}>¨æä2Byü>©H]Œi}?ïÿàŒ"i>êÛ2´åT>ït"ÙJöd>êÛ2´åT?ïež)?«x¹¶UÎ$?"_Ì90 ?«x¹¶UÎ$?ïí"ÔÕH¶?u?ªØ¸Àµ?b{+JS±¾?u?ªØ¸Àµ?ïÿð@¢åü>à8†¤¼\Á>ß~¦\E–>à8†¤¼\ÁAGN3FGL J0115.7+0356@`Ѿ ºKÀM0¶ßû}ºÀ9	ÓöeÀ;xÃkúúÞ?³©ûæ"°Å@[Î\ïÅ@ñÌ )–&¿ÙÊ.Ýc¿æ€=Ÿj5¿Û°üýl&ð¿âþ3¼×?AGNbll@"†·€4mÆPowerLawPMN J0115+0356?ïþ€ö#w?#ŽGd\«(?'ðš|! ?#ŽGd\«(?ïÌà'"æÏ?'kƒ§Wõ?yì"þ´³?'kƒ§Wõ?ïÚm :ª?s;nS
b0?rÉvfó®Ö?s;nS
b0?ïã''¶Ã˜?T›¸äª½m?lØnb/ß?T›¸äª½m?ïý]ðäS?4Ož"'»Œ?5|\Äg~?4Ož"'»Œ?ï-dªN?°YkqI5¬?šSj­•Fp?°YkqI5¬?ï¾øÀ4|Î?…$TÏ?€AÏò0ày?…$TÏ?ï)ØÈrcä?ˆª`§Åh?šÄæé}~?ˆª`§ÅhAGN3FGL J0115.8+2519@`;[ߏG0ÀB›dÜY2À9ç
¶<À;aìNrSÚ?á«ÊžŸ=@Ù»$Ù©)?ÿÊW!O!¿åޛâi¿às݅+Îe¿ß>ß)×Ðó¿ÔkêÒÏνAGNbll@ ÎÖ_Ø­¬PowerLawRX J0115.7+2519?ïþ1ŸÆj™?#Ñò\fÉ?,æç–Ñ#?#Ñò\fÉ?ïˤhL?½X"ÿv¤?z-ËÒhMŠ?½X"ÿv¤?ïéÝ»ÿÂe?lsðQ¤÷?f"DýK?lsðQ¤÷?ïãoô™?PCl¬r¯‹?lp†'?PCl¬r¯‹?ïý	uʇx?3æO4¨ÄÌ?7´R­
cŠ?3æO4¨ÄÌ?ï3$œ¹Öó?®SyvNëê?™›lc· ?®SyvNëê?ﻬتjf?‡mÍâM.?ÉÒMÀ?‡mÍâM.?ïU®Ý'M?''^$ð´?•J$X¨L`?''^$ð´AGN3FGL J0116.0-1134@btÀœ<âÀRZ?ßéàÀ8ê`ão¦À;¬\ê½?êë5·¶©å@®!èÝúr@ÀPÀ6çH¿Þ.ëlcð¿ç´Ak	¿æ¡g"âöZ¿èRàÄjAAGNfsrq@†,AâXOLPowerLawPKS 0113-118?ïÿ:½ì	S?è_ptß?¨J‰ÿô?è_ptß?ïÕÃ1?‡l÷¶@ª{?uquZ?}?‡l÷¶@ª{?ïÅÚ
*®Þ?vxælð<?}úîÈ?vxælð<?ïþDLÛ­?Iõ°´.€?+»:¬$UJ?Iõ°´.€?ïþ ß´+?&Y¨¦Év5?%òã›54?&Y¨¦Év5?ïcØ`Ã~?§è`?õ}?""óÞù9?§è`?õ}?ï5u%ún?"A)¿6Ï?™]Ñ`h4?"A)¿6Ï?ïü½`¦¼u?1ûf&ä­o?:ù6_?1ûf&ä­oAGN3FGL J0116.2-2744@k–PÉSœÀUM`#UÀ:jâÌéRÀ;ñ[dR?¡ZT¤
ûu@
—&`çÌX@.ÿ—ÐA?éÄ×Ä]Σ¿ÞɌráì;¿äƒT¸þL¿Ó¦ýÇãÑCAGNbcu@£õšáG®PowerLaw1RXS J011555.6-274428?ïýSõ ?K°5%,4?3}_þRh¦?K°5%,4?ïÌfWÑx?'Ÿb€¨²?yÌ·è´ëÍ?'Ÿb€¨²?ï¶3©áÌt?}*î‹6?'sƒdé?}*î‹6?ïò·¥sA–?G/ÆsĬC?Zµ -ƒ?G/ÆsĬC?ïú¿»[$-?E	'Œ-Ì?EÑæ?E	'Œ-Ì?ï?¥Èã|?§¡.ª¶˜?˜FãœÐŽ?§¡.ª¶˜?ïjïá`ö?ŽÇ!´;Ï?'¢Ù%,?ŽÇ!´;Ï?ï…uõ¶·?ƒ»ÉXôÄÖ?Ž¼b{³B?ƒ»ÉXôÄÖAGN3FGL J0116.3-6153@rœû`(^ÄÀK~'Éä»À:ѵiÙ¸À;å€~?¡¿©M -Ì@¹"x˜B,?ÿd¿9Ú¿ÝCbB"#¿ådá¸['¿áuÎw¶‰®?"%µy҇AGNbll@¤î8Që…PowerLawSUMSS J011619-615343?ïÿhûc…ƒ?D…èå;?à"Šp‡e?D…èå;?ïÔ!óDÛ§?ŽjkàwT?uï=Eؕ?ŽjkàwT?ï鶄ƒTU?dd(‹öÖÿ?fI{'+
¿?dd(‹öÖÿ?ïþ!#J¢?²Ãð
Ãs?-îÕj×8?²Ãð
Ãs?ïÿjêb<"?§1*çmD?¢±Ô¤‹©?§1*çmD?ï +qGëÒ?³aŠóL?›ú'Ü)ïº?³aŠóL?ïÖ÷ềæ?w»ñ.í-‰?t"
¢"õ?w»ñ.í-‰?ïí™0Ƥó?[jœÃÆ?bfÏfµä¤?[jœÃÆAGN3FGL J0117.8-2113@e:Œ¿+#šÀTdŽà3·À9Is§—‰À;>e§#ÅØ?æj³Æ§ªæ@Ÿæ:@"Áÿê0‹?ÈÞ÷5šÛ¿çpws¡YÏ¿ã¥yéï¿çKÓ µ'AGNfsrq@˜Clô!-PowerLawPKS 0115-214?ïþ¤UŠK?%—'c¾Æ?%º©tR¹?%—'c¾Æ?ïÌ&ªlXK?Ž×^Ñ:¨o?y쪶–
^?Ž×^Ñ:¨o?ïÁ@Š×ë?~xA¿*1?_ºý£ÎŒ?~xA¿*1?ï†q'O´"?jHãN9Ž?Žc›o'zá?jHãN9Ž?ïþ»¨k?,p™/8j;?."P
Ð6Î?,p™/8j;?îÙ1é ÜÉ?³¿Ãc$d$?¢láfÎt?³¿Ãc$d$?ï:´÷ß?"`³ώ:?˜©aVv$?"`³ώ:?í­kd
Vç?"$
'I'?²"¤áMÇ?"$
'I'AGN3FGL J0118.8-2142@e¬Ø'tÀTorßñl¿À8HK"bаÀ;ô3C#k?ûÿaw>Oò@½ßtWj@š*ôw¿â¾¯CAk¿ä֛:…¿äá§fz¢!¿éþœJwÈAGNfsrq@'z¥ãSøLogParabolaPKS 0116-219?ïôÙۑ?U1ñŸT™?VMçݨöÜ?U1ñŸT™?ïÂüpö¯—?‰iD0>]Ê?~ÇœµxŠ?‰iD0>]Ê?íâðj?¢TaÏOtb?°ï/盧?¢TaÏOtb?ïWÙä(£?y{I-5ºA?•ޅ2¹¤?y{I-5ºA?ï®wxBÃ?…¾9îy ?"b!õրà?…¾9îy ?îÎ̏DV?·A)Læ?£>ö/ӟ?·A)Læ?íöxÓâ|?§©~U?·xL:<Ó?§©~U?î¿ðØ®ê?–D)@[W?¤ò'ä­[?–D)@[WAGN3FGL J0118.9-1457@cl O*àÀSt`$-À:Q¹  À;Ȭ¶¬Ï׿º[Ï@'âã@
]7Ÿ©~?ü"Ëÿrfz?ïŠeöÔÞ¿á†áÖÃ-¿ÞœÎ¤µ¤¿²8}4‰¢AGNbll@¯à
úCþ]PowerLaw1RXS J011905.4-145906?ïÿ%îM?¬u$eÏ?B5áF"?¬u$eÏ?ïÑÝѾ	w?;ú›ÖÏt?w<Ôº?;ú›ÖÏt?ïÏÖ¶ŸR°?y*üÁû?x¤³X?y*üÁû?ïü¹im¬×?(Íeį?:4³†QeL?(Íeį?ïþº`—"$?#ËZDæ­?$Yòøߤ£?#ËZDæ­?ï^¬Üu?¨ê©Úe?"*dv"é?¨ê©Úe?ï¶1Ü,Lu?ƒ@ϑ?Þ]?'sˆÿ"¬™?ƒ@ϑ?Þ]?ï굌Ù¯?]%‰p¼^ ?eJs~±0?]%‰p¼^ AGN3FGL J0120.4-2700@j²¸`™ËÀTáþ@_ŠÀ7âW5ŒªÀ:ÙP·¨xZ?î¯Xº@-•'ÎÏ0?þ E?z>`¿ÛôxÜÏh!¿àI€4ߛ¿Ú>«<7¿Ýï²!r7øAGNbll@—ÌFsØPowerLawPKS 0118-272?ïû'#†ö\?;•õÝò?A»qv3Õ?;•õÝò?ï²."Ó¹?"ÝeP…·6?ƒtwMJÕÌ?"ÝeP…·6?ï:jفá?•;¼©´1?˜²¤ÈðËå?•;¼©´1?ïj³°¤¬?"1QŒ‡³Î?ŸR©‹£8‰?"1QŒ‡³Î?ïøG'âv?Møà;3¿?Nḻ&r¿?Møà;3¿?îKÃSbŽÒ?¶ÖI8?«CÊˎàã?¶ÖI8?ï }ódªé?–eä:›•?›ðAŽC8à?–eä:›•?ì!ÖfK?§@šÙBxŒ?¾ñLͧ×å?§@šÙBxŒAGN3FGL J0121.7+5154@_ìÀ§¨À%_tÿ†]}À:›=އàÀ;—f=Kºé¿êz¸•)¿¹@
7¢wŽ¬×?ÿ¾Øà×EÍ¿éîÃà—´¿ÐåI=ê#þ¿Ò‡­rOº¿èƬªËúAGNbcu@ª¾EoPowerLawNVSS J012133+515557?ïü²ϛ½?7›ý›z†?:oéºÙË?7›ý›z†?ïÂ*⬲ü?Œ²­'R×É?~êŽÁÙê?Œ²­'R×É?ïÌèÌÔ0?zÙÄF‰XÜ?y‹™ÜI"a?zÙÄF‰XÜ?ïüߧDýá?)8"½–?9Ɯàýö?)8"½–?ïñ~+^~?[L)CY<Ð?]ª.:C©?[L)CY<Ð?î¹$¦þ\?³§[6?¤mµ"eÁë?³§[6?ï•äT0V?‰­¨ŠÇE"?Š†ë
2Z‡?‰­¨ŠÇE"?ïÚdñ­h?kÂgíôÀ?r͇ÍÖ1?kÂgíôÀAGN3FGL J0122.8+3423@`Hüàü.ºÀ<€ÌC:À9ò¯ñʳÀ;x¢?Zˆã¿ð–G²œ@
]Œ©ÇG?÷Áˆ`Œ1Ò¿ä"ÉÑ¿áÔ÷p0áí?°DS½¨}É?²žçóUAGNbll@èÅ?|í'PowerLaw1ES 0120+340?ïþb®Bj€?)ÜAï?'±?)Õk'è?)ÜAï?'±?ïÌòáMQ0?Àf*?y†U7ßÔ?Àf*?ïÇòˆ–?†IˆÂÙDZ?|ü½»ô?†IˆÂÙDZ?ïÿôA…ÜM>˖F•&fv>×|—ÛOãe>˖F•&fv?ïþç$j?1) ®¼Pú?.qŽÒZ@?1) ®¼Pú?ïcƒòàª?¦W
¹þz*?"©&?¦W
¹þz*?ïÃ1zmÑ·?"ŽKOoæ?~gBÒ l?"ŽKOoæ?ïÿ» ãÜ>ÿ"2ïαÀ?7ñ"€¥>ÿ"2ïαÀAGN3FGL J0123.7-2312@gMó`Iì³ÀTmŽõƒ¥À9¤†ü#»À;ž_7ûÿ?͈–'ôø¡@'@'m€?ÿÐ1€Ö(¿êIÒ¿U¿É|ö«mŽ¿á©}~ÛÓ¿à+aé©ýAGNbll@¢ÜzáG®PowerLaw1RXS J012338.2-231100?ïÿ+7wvÀ?©¸õg¬˜?™Nå²ï?©¸õg¬˜?ïÏ9ú€Aâ?'Ï,¹Ì‰?xcˍºÅ?'Ï,¹Ì‰?ïæydM	?cH†ã#ÈQ?i†›–óÑ?cH†ã#ÈQ?ïÜ|3=€O?Uc"íž\*?qÁæXPÜa?Uc"íž\*?ïýë<=aÏ?(â¥SB'…?0¦ -Q.?(â¥SB'…?ï#/sÏÊ?±àå~¤"­?Ûš­p°?±àå~¤"­?ï½(
qYE?'×Í] ¬ú?€µýSÛzâ?'×Í] ¬ú?îÛPq?l?Œ«WšR›?¢JøìxTI?Œ«WšR›AGN3FGL J0125.2-0627@b6"_õIÀPô'@.Ä9À:6¼ÿÐ/XÀ;×ÓãAƒX?ñGFÐôÏ @SU=õ"@©Ë€qt?ïj6&<D¿åĬ…%Ë¿æÇùG^'¿çƒ¬þPRAGNbll@"¾rþÅm]PowerLawPMN J0124-0624?ïæ1"(™Û?'³Rä߬?iÎlîÃ}%?'³Rä߬?ï9ò,á=%?ž5û=JÈ?˜ÁºhÿÅ^?ž5û=JÈ?îÑ£,%´?˜vü]r(?¢åÍ;ìò?˜vü]r(?íeïr‹…&?"µ…¿OÈ?´Ð"jÇïÏ?"µ…¿OÈ?ïærR'Ùº?xí-x/Ó?i­8nÅ?xí-x/Ó?ì	¹ü?À"Kš»¶?¿·z7 '?À"Kš»¶?êÕaìâŸ{?²H¹pŠ¾?ĪxLu'?²H¹pŠ¾?åŠÌލÓ?¶óÑ)-í?ÔêftÂäZ?¶óÑ)-íAGN3FGL J0125.4-2548@i ½ ßÞøÀT''?àÀ À:Œn7ìÀ;ãKÊíñ?ä)ˆ[òð@pÀþãJh@	läÛ¿æÉ "ì¿Ö±yJÕÍc¿ãPÎúyƒ¿çBӃdçAGNbll@˜kÙè>B[PowerLawPKS 0122-260?ïÿÓPZLj>ñd<njF>öWÜÛ:·>ñd<njF?ïÌéø¬¤Ž?ŒÆw´q«!?y‹Âjè¾?ŒÆw´q«!?ïè¾N?o\tÚ!f?gA±ÎDP?o\tÚ!f?ï¶ü#ºð?aÛÜ"
?'@ýõø?aÛÜ"
?ïÿ‹[=hk?Ýq\ônT?
)A©¸pô?Ýq\ônT?îëòßÛó0?²T÷OÑÚ?¡@Òˆþü?²T÷OÑÚ?ï×kl".Ï?yX'AÖl?tJI¦šd—?yX'AÖl?î[ƒ"¨ Ï?'µƒ'Ú?ªGƶYÚ?'µƒ'ÚAGN3FGL J0126.1-2227@g)Ÿ¡—ÀT6· ÝÞÀ9'r#3
ïÀ;§èÂ̙?æz–oÔµ`@Ĉ;Î7[@q'Iüο×:A؛Ì¿ä¹-ÔW8T¿ê˜mhÒì¿ä>»×S…ÛAGNfsrq@‹*dÂø8PowerLawPKS 0123-226?ïÿH_•;ç?ÿ'P¬v?ôü?ÿ'P¬v?ïÓþ%ùþ?‡^E™z+?v~€ÐÖ4ë?‡^E™z+?,úR?†ÑRR=ü?ŽP´æ`£'?†ÑRR=ü?ï֝Â.tn?Vß/jn»L?t±îõ?Vß/jn»L?ïþ	¯Œ+?5Ù©&ê¶?/ey©,¥?5Ù©&ê¶?ïÖvÕÛz?²ò¯àŒ?œå1eX»?²ò¯àŒ?î²nCÌÕÓ?—ןÕ/?¤ÙÀžíÌ?—ןÕ/?îù¼´i)?Œrl'¼? d?CŸw?Œrl'¼AGN3FGL J0127.1-0818@b—ן#FVÀQWü€¿À9§¨Xy=ÙÀ;»ŽÐû«?ç¡J/¤‡@aé;îB¾@²ãàÈñ¿ãŸIÎD

¿áGk#|4¿æ÷Û\S
¿áNL•AGNbll@'šrþÅm]PowerLawPMN J0127-0821?ïü»h±M?A[XÇ 0?:'…éì°c?A[XÇ 0?ï¹Tq5;:?*.:<?ªã¹è_v?*.:<?﷔gUm?xŸ€ÉØ?'æ=ê¤Ø?xŸ€ÉØ?îç/éÊ?€â0ê·!?¡`ÌJP?€â0ê·!?ïíS"kv4?fþËÕ«?b¬k ècp?fþËÕ«?íu02¸#?¹V­—Ň?´V~q2ç?¹V­—Ň?ð"•7?_ÓhM0?¥—€ô2÷Œ?_ÓhM0?çÉ¯ø?´[öãÜ?ÐÞmÍÒ ?´[öãÜAGN3FGL J0127.2+0325@aƒ&€IRÀM ªKÀ9LntQátÀ;hŒ'sZk?Þ8
(Lû@9rƒ«Ë?þce€À?ײÃ%	À¿àPxµÀ¹¿Ó҂4^g¦¿âÔWC~†AGNbcu@¢YRòäPowerLawNVSS J012713+032259?ïý''ò¿?.Zd|G[?3kiš˜~Q?.Zd|G[?ïÊË7ÌJ?‰÷l飼?zšd8'U?‰÷l飼?ïÔÀ±-Œ?p·"ì<l?uŸ§Hƒzg?p·"ì<l?ï¡-[F¼l?gYȈñ[ò?‡´©50?gYȈñ[ò?ïø8·á¿?JòÕ5Ǔ"?Oø½"C?JòÕ5Ǔ"?ïV™ê¢K?±CÒüÊh?ŸÕ,ÇÓ  ?±CÒüÊh?ï®Ý‰Ä •?"Óº%?"H™&®Ë?"Óº%?î\iÇ]»â?Ÿþ)êsÍ?ª9cŽoÄß?Ÿþ)êsÍAGN3FGL J0127.9+2551@`£ýq?ÀB%'Éä»À9¥Z'"ÃÀ;§YE³Æ?Û
ZÆõó7@­wt«¤@Ìc¿˜ñ¿çÃ&$Ö4¿ë涴BÎm¿ïÿì0€É¿à_ËÌ5'÷AGNfsrq@nGZ1¤¾PowerLaw4C +25.05?ïþ´¼hY8?/÷¿¼?$´9zlz?/÷¿¼?ïÅ,¦7rï?‰ —EɑC?}i¬âæ°t?‰ —EɑC?•¹2?‡ÇV™L?‹•_ŒÓC§?‡ÇV™L?ï‰ÛRT?uSý|CÒ¦?‰:á.Vö?uSý|CÒ¦?ïøì¬L_æ?RϫؾL?LMOÊJ,^?RϫؾL?îôœ8t*?µþ¶·¾"?¯0¶>0‹e?µþ¶·¾"?îޔsÑI?šÚfîj?¢¸Âîkr?šÚfîj?édHC]X?»7"6 rs?ÊnÞò‹š ?»7"6 rsAGN3FGL J0128.4+6257@_È
€CR?ÙØÀ1D,À8õeQ"qÀ;:-"wú?ì†ëÚ.4F@¯çcÑâ@	/ÿw¿àgÉ<õT¿åÕ=Ÿæ@¿å†ëabpŽ¿ïÿ‰OTHERspp@…‰€²BPowerLaw?ì0Ž¥l-?¿‡‡É7–ð?¾{ŠÔž—?¿‡‡É7–ð?â¢ðÞ¤æ?Ê@":Èäò?Ú»âB¶3?Ê@":Èäò?êñcžÏ¨?®/Uëuz?ÇÀ:q"Á_?®/Uëuz?å#;M!à"?£Q'wÀ¶&?Õ¹‰e¼>×?£Q'wÀ¶&?ßìõ"·Ï²?Ð(–?O©¿?à	…6$'?Ð(–?O©¿?ÂÐΏ•?Äö²Ò?ëKú~œ?Äö²Ò?܂­Îs¯¿?¼˜mxî9?ᾩÆ(!?¼˜mxî9? §U?›°"S.Sº?ëWà*¹½?›°"S.SºMIXED3FGL J0128.5+4430@`;ªÁ	J,À1݆ÀytÀ9ØÊUú˜À;Âٗ¶j‹?Ʀ/UÔ¦@ø|ôGe@¨À^Tt¿ã9\ZÒg¿ç™ë 02¿áۘ=_BA¿ë–ÞûðÉ#AGNfsrq@
\C,¥zPowerLawGB6 J0128+4439?ïÿPz–Ê?©™Y1?ð¦2jé@?©™Y1?ïÄ4«`ôë?ˆSrõj%?}åªk²VX?ˆSrõj%?ïÍAÁTÁ?q.Îz}?y_u/Ó¿r?q.Îz}?ïï½åX?A¨9õ|'B?`BáÞû 9?A¨9õ|'B?ïÿJ;7? Õt¼Ü?v³ß—´û? Õt¼Ü?îñ"ÿ"NM?¯Eß=Û? íÐ
k/?¯Eß=Û?ï¹ëÜåý(?'ÚjmÔ¾7?…Ï»ð?'ÚjmÔ¾7?ï•Ž»!Ý?x2TT5w?ŠºœCyÉ?x2TT5wAGN3FGL J0130.8+1441@a Ç`|ÀGšÿË&ÚÀ:5O•GûÀ;Â+,Ôta?éÈŒZÒñ@ˆaq´ù@4NŸö*¿àÁÄ¥®GH¿ë¿ì¡ÿC¿ïb…¤ÖIß?êal×n¼AGNfsrq@€ì'£S&PowerLaw4C +14.06?ïþÆ@Z|è?.$î ?#›ù®Þ[?.$î ?ïÎ-±­ÑN?!Y?Wþ?xé')Y?!Y?Wþ?ïizú¿p»?Šè	+\V?'Р«"—?Šè	+\V?ïúÌc_9»?BÚÐ}cn#?DÎr¦Õ5?BÚÐ}cn#?ï÷h›:¹?cxi'FÏø?Q.ÉÄ/?cxi'FÏø?ï<Yš?²}øiJÖÅ?žl[¾"Å?²}øiJÖÅ?írÇlÝñ/?©Ÿ
¹ƒ?´iėƜ?©Ÿ
¹ƒ?ï"iì­½¾?K')×¢?Žå"Ñ ô‹?K')×¢AGN3FGL J0131.2+6120@_ëğס<¿òµQ€¦-§À8w3¼ÅîŒÀ;§' Ö9¿ëëQÑ?3ƒ@êÍ–*y?ýÊ€¥+ô¿àÈSõlö¿â~zm?¯ª¿Ùq¾óŠ°¿Ìsì.›AGNbll@°½È´9XPowerLaw1RXS J013106.4+612035?ïÿžcáY? âŠû ?g9	 ê? âŠû ?ï¹&:¸sá?"@rd`"?¶qKÏç?"@rd`"?ïÏñ\ªs?L®aèS?xRג…?L®aèS?ïÿâ(Ý!Œ>å…ÙÈ3¹J>í×À+Ê£>å…ÙÈ3¹J?ïþQ`,?,Á»3cß?*éüÌ?,Á»3cß?î"&=˜p?´'Á1ósÿ?¦Ížü&y?´'Á1ósÿ?ªSå?"I+ì?‡˜•uŽ·?"I+ì?ïÿSB$ñ?µÿÝZDf?Փ6²-<?µÿÝZDfAGN3FGL J0131.3+5548@`οìºÀƒ<ŸÃFÀ:=0l¯VÀ;šºZ•¿ñ7`Ú5k@kÏæ1Í­?þv3þµ'?¿ëΐŸ‡¿Ý€Òõþç¿á#qKòœÀ?¢ÔoÁAGNbcu@µÒîBZîcPowerLawTXS 0128+554?ïþøԛ*ò?™WêÏ? r´Ð⋊?™WêÏ?ïËÝ#12}?ƒŠB?ëÕ]?znˆcR?ƒŠB?ëÕ]?ïæŒ}¬G?bÜ´Ëø??is'±[9Z?bÜ´Ëø??ïÿî­r>Œ>Ýhè‹"FR>áRˆ¹«7>Ýhè‹"FR?ïý$¹¦\ÿ?1¡ô$L¥?6Ú2NB?1¡ô$L¥?îæ-võo?¥ÀåÔSÖv?¡ž=(©?¥ÀåÔSÖv?ïу'
þ?vþi$KVÈ?w>6Ü?vþi$KVÈ?ïþàR»Ž·?"‰'תý?!úÖxè—?"‰'תýAGN3FGL J0132.5-0802@bûw µíÀQ%4ß۝JÀ:ˆÉûaÀ;¸A›«Â'?à :M·³@óˆzãK?üÚß_ ¢¿¶S"F@g?ïšÎãõ«¿ÚÎOT¦ö¿Ðà-ëSSBAGNbcu@±$Ý/PowerLawPKS 0130-083?ïþFεI?*'ú¢=?+"‹æð?*'ú¢=?ïÅÓé÷ÿ?Œ3šVðâ?}_ˆ›?Œ3šVðâ?ï¡»ˆúŽ?ˆE…ÕžUâ?‡'¾Ày?ˆE…ÕžUâ?ï˜JÝ\?q">TÚ?‰í{þZÛ?q">TÚ?ïùïxÚm…?K27xÒУ?HB£«HŸ?K27xÒУ?îÚGG£há?²Œ[{Miš?¢[‹'YÕí?²Œ[{Miš?ïy†%m»?|µª"´J?Ï;c™²?|µª"´J?îm¹&?œkœ2œã?®o™1h"–?œkœ2œãAGN3FGL J0132.6-1655@ed@ò8—ÀSÁýaÀ8]à_PÈoÀ;Œ­Ánʹ?ïj
®ÀÙ`@홟£ÉÉ@pê¿üÚ²¿âðƒÑk¥¿æH @ÎbŠ¿éQØXNÔ¿â—!B¬BAGNfsrq@ðØDÐPowerLawPKS 0130-17?ïÿo}Öz?M@ʯh:?MDzÌ?M@ʯh:?ïÊí¡Ú?'ÊÏ)oüA?z‰uñ/ù?'ÊÏ)oüA?ïÂ^õ-éó?yƒ	5?~Ѕ`
{?yƒ	5?ïèªzm?OÄ­ùèˆ?gUäˆ2B?OÄ­ùèˆ?ïÿA'¬[,?èôr2â?Û	*OhÓ?èôr2â?ï*¾9ó'?°ð¦yòw?š­è:yi?°ð¦yòw?ïpg{å(¹?l±FCB?'óŠ: Ð?l±FCB?ï¢w™iþ?{é
‰?‡b¯çT\?{é
‰AGN3FGL J0133.0-4413@qy[À6ãÀQ½²_Μ±À:/ĦãÀ;üË+­-¿äP/5€H@@$³=°@?ü¿ÙŸC¿Þ jpX¤ÿ¿â~U<ê¹i¿àÈÇL/Xˆ¿äJ‡áò_AGNbll@–Å7éùrPowerLawSUMSS J013306-441422?ïÿnhψz?)óž$¡r?2í[«›?)óž$¡r?ï×ëÆìR?‡…ýͤ!Ù?t
9Z‹?‡…ýͤ!Ù?ïé‡ôÃP?ZÑ"‰Ñ?fxìºÐ/?ZÑ"‰Ñ?ïýˆ[ƒ´?%‰ÏÇvb«?7¼$Ì+‡?%‰ÏÇvb«?ïÿ˚ÙÇ?j£ú‰?¦'Æál?j£ú‰?ïSÞ40ç²?­ùÙ ¦?•"9vsmÄ?­ùÙ ¦?ïΑ¬v|D?|
ߜ÷1Ñ?x·)¬´™ô?|
ߜ÷1Ñ?ïÛ
E[ÝT?fHÎ멒?rzÝ[Qî?fHÎ멒AGN3FGL J0133.2-5159@rˆv\ÀOö¸¿ÏŽHÀ:pƒÇ ="À;î£~éпÔâHæ_R@õö`X@kŸ`X¿êu«Èg¯´¿ã8c‡'Ç¿íÁ5
—±ý?ØJÛ~SÌAGNbcu@…cT`ªdÃPowerLawPKS 0131-522?ïüÞãþ ?Hñ¬|ÈE?9Eb\W?Hñ¬|ÈE?ïˈZW?'–p/Ã1?zwü¹$}?'–p/Ã1?ïb¡OÆf×?‹¨cJ¢ò{?"«ÖSí%?‹¨cJ¢ò{?ïÿô%ù†?ĪJºU¸?Âéa'ë2?ĪJºU¸?ïñý?J1–?aÂ0´LQ(?\êrÓ?aÂ0´LQ(?ïR»¢
´í?¬šÆ_2[?•¨‹ÃÐÌL?¬šÆ_2[?J½4÷?™c7Ï«ù?¥¦ÛP½›?™c7Ï«ù?ïõpðᇢ?X6þh¬	?Uïù{m?X6þh¬	AGN3FGL J0133.3+4324@`^œŸr÷nÀ2Ш߇ºtÀ:BЏ±¹À;Ԓr]ën?ÞÁ4]·ñ@¯ùO·£@h~€
¬f¿Í´›â&Ú¿éM$ÓknÛ¿áËÈ­zÄd¿æ9'%y-¶AGNbcu@"žïiDg8PowerLawB3 0129+431?ïþñ
ªå?+B諓›/? ïXïyÒü?+B諓›/?ï±ÌñVå?'ÒùB¿?ƒŒÃ´Sí?'ÒùB¿?ïÅ}å«bf?~uüƒa/ƒ?}A
*þ¸Û?~uüƒa/ƒ?ï©@÷I«£?b¨ý–÷?…¯Â7ãë#?b¨ý–÷?ïûŸ½†D?G­¤àž¿g?C偩q?G­¤àž¿g?î5Ž:Ñô:?°Œ­O×?¬§N•9c?°Œ­O×?ï H<ð:?•œÂ»Hbg?›öïÚƸ?•œÂ»Hbg?틬•"?™8SŠiñx?³¢›XE`?™8SŠiñxAGN3FGL J0134.3-3842@p¾àP7PÀR×"Àh¡À:E©¸ËŽÀ<jüY'¿è"íŒò@tM¿%šC@¦H «L¿æâ.ÝdÖ¿æÚešA=¿Ð·½å4¿ëøÎEGݺAGNfsrq@q6âëPowerLawPMN J0134-3843?ïúсVE¡?Cڑ÷ïa?D¹úùìÙz?Cڑ÷ïa?ï×wŽxv?ˆ9Ý£2g?tDqœ–ùR?ˆ9Ý£2g?ï"Ö¤Ô?ƒIgåÝãø?ŠÊVøJ¯?ƒIgåÝãø?ïþ~§-l?øÁЕ ?(Œl}\?øÁЕ ?ïùõeƒx¬?Q+óÄ~Ô?H*iÝÆ?Q+óÄ~Ô?ïGùóÂ?­^ºr¤«?—߈m´?­^ºr¤«?ï…Cá"¼?‹"}*A*?Ž¯ÁŸ¯ú?‹"}*A*?ïôp¢nC?R6ŠBq??WÁ&WHä?R6ŠBq?AGN3FGL J0134.5+2638@`׃¡	ÐcÀAŸT_Ó¥.À9bÒX'ƒÀ;{"qê('?ñÄmO¹¦ª@>¿Ä¦Ž?ÿÛg_4Ã×?ÑEÉïˆõ™¿Ù؀	O´ô¿ÝTžg½1¿æí¤èFÏAGNbcu@¡µÜÆ?PowerLaw1RXS J013427.2+263846?ï͸Òfa*?t>Xò\ÃÃ?y#–Á ¾á?t>Xò\ÃÃ?îä‹Bè?Z{0(åó?¡·Oz 3z?Z{0(åó?ïÓX{?"ÿ
Ø(ø&?%ðŸ\?"ÿ
Ø(ø&?ìu^XrTS?Œtïf
é?¼U
<m]j?Œtïf
é?îìQ£-Ë?¡^å/ówV?¡:î²]‡[?¡^å/ówV?êÓÌI³ìñ?ÀŠÊOU8þ?Ä°ÎÙ0L=?ÀŠÊOU8þ?êÇkÞí®?±þ'ÉÀË?ÄâP"IG¿?±þ'ÉÀË?ähÏWŸ+Ý?§V3B–‹D?×.aPÁ¨E?§V3B–‹DAGN3FGL J0135.0+6927@_°ÄŸ×¡<@¬Æÿ®K'À9ºGº©´šÀ;O‹Ëz½?½I¢z,°§@Ó.ö¸ƒ•@tcßÎ\D¿ÊIÅëKô¿ëÂsÊý꧿å¾ësè¿äU÷i"ªAGNbcu@‹£S&PowerLawTXS 0130+691?ïø(R&	÷?Y›xÒ[Ð^?O^¶ø>m?Y›xÒ[Ð^?﹨øS°¤?‡FU5!Ü?•Áêõ?‡FU5!Ü?ïDü@ظ=?ŒϤ_É©?—`wÜQò]?ŒϤ_É©?ï²w*Ñ1X?e½¨«Ôv?ƒb5WºKø?e½¨«Ôv?ïº5ºÎß?ˆòæìý|•?r'Uœüe?ˆòæìý|•?í·T.VL?¸%¡©	X?²E_M ?¸%¡©	X?í`âvd?ª,ò"ê2?´øìQ>ºe?ª,ò"ê2?ìLý®/ír?¨êc&9&r?½˜Ž€"n?¨êc&9&rAGN3FGL J0136.5+3905@`9à`þHÀ6ñ§Ši{À7p͔ré,À:sˆ¬Œ%?çKÀÌþÓ@‡&°:?û!/à˜[¬¿á:p'2¿×ᾨ·¿ÒËjµ^#Õ¿Êþô^®ƒƒAGNbll@£ÎV»˜ÇãPowerLawB3 0133+388?ïð"pxÊ'?]<±mí	«?^÷¥÷'Ã?]<±mí	«?ïÂÎðm?†2"*æø6?~˜ÿ~†?†2"*æø6?ì"ÏF
®?ªÔÄÛM?»Ù…ϯ¢'?ªÔÄÛM?ï¨ÕZdi?náVðÈB?…Ê»ifå¬?náVðÈB?ï£yJ÷†?‹ÔQ,k¹?‡!›âóJ}?‹ÔQ,k¹?-óêY?¯çB£Kp­?¤·ý ÁZm?¯çB£Kp­?íÍ´×ô¯P?¥yÝ'Â?±'Y@Èxþ?¥yÝ'Â?îÄ÷}%?˜=¼$?¨¾Môxº?˜=¼$AGN3FGL J0137.0+4752@`Yi ­ŠÀ,˜¥ÀïHùÀ7²MryšÀ;ªÆè‡=?ú"ç÷²@WK@î>¿àä-R.Ý¿ä¢jT¡[Ê¿ãùÁˆ(¶‹¿èãÅYÇ¿AGNfsrq@€YÞÑ·LogParabolaOC 457?ïøå}À?RÈ_dEx?MÈiê?RÈ_dEx?ï½õpJ¸?ŽøMœ$•?€'¸¢åoö?ŽøMœ$•?ïwô¦¹q?Ž10Þöï+?'k/»é×?Ž10Þöï+?ïõíõçMW?>æLF	R?T$»2Ãd?>æLF	R?ïælݒ±?oô§n…Ïü?i"";Ô€?oô§n…Ïü?în벸pí?¸y«¿@Z)?©DÖ0¿4?¸y«¿@Z)?î´ª8š?x|I™Õh?¤µ\r
£6?x|I™Õh?ïõ*ŒÏy?OÂÐa¼9?Uªæ_#]É?OÂÐa¼9AGN3FGL J0137.6-2430@i,ÀÒÇÀSÑÒtwÀ8柱mÀ;ÀØi¹>?ﯟ%°ÏÒ@ŠVf/]@$ Tä¿ã@ÎØk~¿çCAj¦¿éi¶¼Xû¿ç¾ãèÈ*ýAGNfsrq@·XâPowerLawPKS 0135-247?ïÿ~¼Š?ûç½ý…Ý?>ée°?ûç½ý…Ý?ïÏb'xß?ˆópv'C?xN¿p\?ˆópv'C?ïÎcÄ÷'?lÜñ¿?xÎ}¦tÇ?lÜñ¿?ï®SŠ
,?g1¬©ûiS?"kŒƒ2±?g1¬©ûiS?ïÿRi¸?C츤FZ?²ÙÕ(ïÇ?C츤FZ?ï6$ÈÈl|?¦k!^üd?™;fÞ[jŠ?¦k!^üd?ï´n³«­\?x¢´»€?'äS"ì?x¢´»€?îoH¢'ª
?—ÏØíWáÝ?©uß=-V?—ÏØíWáÝAGN3FGL J0137.8+5813@` Ç1¾À\l.NÀ9Ý:ZMÀ;OZˆ%¿çê3!añÚ@Ü¡jHs6@u8_—ë¿Ú¶½Œ'¿äå?æ'šV¿ÞÁ¤G¿ÜO³7‹˜¶AGNbcu@¤·?;dZPowerLaw1RXS J013748.0+581422?ïú©ñÍڋ??¶½‰"«?EX7Èf't??¶½‰"«?5ƒE«l?Ž߯eyP?€ÚŸ=[vç?Ž߯eyP?ïÂÏLGÆ?|&5ÆûÅe?~˜YôÚ/P?|&5ÆûÅe?ïþ02*}5?/m3ü?À?,üß@[—ö?/m3ü?À?ïñ@e%?Y%a|‡f?]×~¿Á&?Y%a|‡f?î‹îès2?´·áê¿q³?§A€ š×?´·áê¿q³?ï)^%ص?Ž¹;ø"?µ¨s6µ?Ž¹;ø"?ïèÎñPv?`%'mθ&?gr0ËW2h?`%'mθ&AGN3FGL J0139.9+8735@^ß/@_k @8ÇÞàˇRÀ:[o¨.‡ÓÀ;Óác\ƪ?ÎcJ]'@
èO-°7?þBŽ_Ô¦á¿î¿?97z?Ûd˜nSù/¿ã"=êZۿŬ†6́	AGNbcu@²ƒÇ+JPowerLawNVSS J013913+873754?ïÿ†iL[?IPH™Ä?1+ØTo?IPH™Ä?ïÜNüMª?pžOhumÁ?q؁ï(vR?pžOhumÁ?ïá4ûVÅV?jô‡Ýt±Î?nˆÞ'-?jô‡Ýt±Î?ïéLÍcµ?På~ÓO\Ü?f³2s¤û=?På~ÓO\Ü?ïüŠ¿ƒ…}?6p€P\`Á?;ªs}ö-?6p€P\`Á?îßь$;?±Áµó8?¢òè£M?±Áµó8?ïÌ?#3È?wIȘ¯½?yàuÛ(L&?wIȘ¯½?îü}:N–¢?"}ˆ87? 8,[ò|Ü?"}ˆ87AGN3FGL J0141.4-0929@c╁$ÝÀQ19Ü>ZÀ8~ê–pÀ;Rùþ?ÜágfÊ@\ÀÃÕ@ûª ¨»¿ØòvÅf/¿ä1Q÷zÜ¿áh'N4§Ž¿ãÑi—H[ŽAGNbll@Žk!-w2PowerLawPKS 0139-09?ïÿÎT¿Ós>ðVŽýS?œ>øÕ½–™ö~>ðVŽýS?œ?ïÊ0ÔøÚ?'Œ|²æÄ?z畚@f'?'Œ|²æÄ?ïæ—ÈÓ³?iË`Î8h?ihëc'M?iË`Î8h?ïÞ½ùþ½?VÀZ"¶8a?pò¡_9'?VÀZ"¶8a?ïÿÁǓ°>÷äÊ9"z¯>ÿ',§¼Š>÷äÊ9"z¯?ï>·e(ñ?«nÚ(j?˜)\™­?«nÚ(j?ïۍlº"d?}{E@‡ø?r9I­!Ì?}{E@‡ø?ïJjpÐçR?'GïªÆ=?–²±åã±?'GïªÆ=AGN3FGL J0143.7-5845@r'@$³>ÀLŠ+¿¡kÀ9)–‡å<À;h¦©L•¿úÊ+lë:Ì@ƒ§>ó±?ýj*þÜ>…¿Ù²ðm:ëä¿Ú`%¸)¿âðZ›ü¿¥Fÿæ!)AGNbll@¤0£n.²PowerLawSUMSS J014347-584550?ïü¬'Ë`?@ÅYd©À?:›îÇÓ¸9?@ÅYd©À?ï͌žÅŽ¦?'C7ò8+?y9°~L1?'C7ò8+?ïÀ;»ê?ƒJæ¯'Dš?õâ¯5?ƒJæ¯'Dš?ïÿý‡é®>·VŠŽ&t>³Ã
Y¥˜>·VŠŽ&t?ïý'ë3?6	4äJ=à?7ÖÇÌÑÛE?6	4äJ=à?ïK'Êä9?±ü1 ò?–›¥7fÜ?±ü1 ò?ï•n¤a°?‹pI3èŸ?Š¤xÚW0?‹pI3èŸ?ïÿÚû±C>øNlñ^<>ò'Dïá"U>øNlñ^<AGN3FGL J0144.6+2705@a)  ôØÀA%ë`5ʽÀ7ÙcaÏ'ñÀ;a$WÎ?ò†¨ÀþãJ@D8"*@kïð=jD¿àK\øÜþ§¿ã_Š±
Bx¿âÕAVÛ¿ä —YAîAGNbll@€í)Çy¦µLogParabolaTXS 0141+268?ïÿˆ¥šG®?Y«›Å?
Ö£zïæ|?Y«›Å?ïÆãa8Õ	?‰/UiO5.?|ŽOdEg§?‰/UiO5.?ïӒˆ÷z?tßgdI˜?v6ô ·OI?tßgdI˜?®½v?gñ†8Àp0?Œ"½P¢?gñ†8Àp0?ïÿSo¾?5üX/÷?œP}.8'?5üX/÷?ï	'Zì=^?­Ø±àÌÙÄ?žÏ´¤0"<?­Ø±àÌÙÄ?a˜újó?"öè7R?€Ÿ™Å,Õ)?"öè7R?îvne?'ì®a!?¨ž!d?'ì®a!AGN3FGL J0145.1-2732@k>àŸèh4ÀS"2_Μ±À8ŒpUÓq,À;«ô5Çb*?ñâçæٓZ@ýˆšBáÒ@Ž'`:'n¿äs'¹áÁ.¿çódÑfs¿èîÉëਿì(LQ"™AGNfsrq@z.ÿëJPowerLawPKS 0142-278?ïúŽD.‹·?>º÷­mr?EÆðK€.ˆ?>º÷­mr?ïɹ6dbx?'_µ~CÖ-?{#dÍÎÄ8?'_µ~CÖ-?ïtƃ#ƒ?'i¿ÖÖü%?'g?
t%«?'i¿ÖÖü%?ïÖ{e3Á?YÇùCòIé?tÂM2†ç›?YÇùCòIé?ïù'_Š÷b?H<ëlï?I¶'Ñ't`?H<ëlï?ï Ý´ëH?±yKš ?{äLÒ2ì?±yKš ?ïtâIO™	?@ºbðmÄ?'c¶Ù|zÓ?@ºbðmÄ?ïvzevÒD?ÑŪ'??'0³Xïk?ÑŪ'?AGN3FGL J0145.6+8600@^üá~4¹E@7<ö í¦À:@yꧩ'À;Ú|öË£Ø?ÍÏ·úKO@e™
©@&«?ß>¿åL{7-ê¿á¨å¨P¿æØþ"¿æ¦_&oðAGNbcu@‰PÅ¡ÊÀƒPowerLawNVSS J014929+860114?ïýî¯duå?5ü/(ܱ›?0ŠƒîÒ>–?5ü/(ܱ›?ï®Ýz¼V)?ŒÝ°òYW?"H¡M"ã§?ŒÝ°òYW?vs`?|°Üdp?ˆ_¢c'þ³?|°Üdp?ï'ñðõ?|$šÝõÍ?›ÂT¯S?|$šÝõÍ?ïáÖî9Ú?u'ph½£?n)ï6	?u'ph½£?ìXCá+S–?ÁM=͍^o?½=àö¥cQ?ÁM=͍^o?îDqG|&¨?£¨4ÿöw?«¸ë‰|z?£¨4ÿöw?åþ}å;·?¸$ûn?Ô5ˆ'Î?¸$ûnAGN3FGL J0146.4-6746@rqú?̞ªÀHB=ÀTïFÀ:4Ò{bvîÀ;÷õy"@"¿èzjÉfT¸@
ÂPŸªª¹@ )`vP¿ãµ¡Øà׿åFGž¿é=uó»è¾¿Öb¤æåãÛAGNbcu@ì…à´áPowerLawSUMSS J014554-674646?ïû‰~‰º?CÓ°ä:6Å?AÚR*þÍ?CÓ°ä:6Å?ïÛÕ½'Â?€cªï̈?r!Ž"Öµ?€cªï̈?ï¬ý8iº?wZ‡¤f^©?"À¾?¤h?wZ‡¤f^©?ïþMu 4ö?ÚQê"
?+(«'!º?ÚQê"
?ïí­dtH?g,jÍÄe•?bR›Ìƒ_ž?g,jÍÄe•?ïZŠz[Z?«Öàœ6?"®°Å̺?«Öàœ6?îæžx^Ù?–ÜÕ®rę?¡–•
vx?–ÜÕ®rę?ïÖ÷ñ=Å]?p"\Iůl?t"L©f?p"\IůlAGN3FGL J0147.0-5204@q¿?á—_ÀOz-K6À:=ƒJ¢»À;þ0íÖ¿íÊ֗?»ñ@:9/K@˜¼ R;¿Ä¢¾lô¿âð³¡á¿ç†kEÿÀ8
{Œ›ãAGNbcu@–×úCþ\'PowerLawPKS 0144-522?ïü¶Òd'O?>N!]Ú\?:Inä ª©?>N!]Ú\?ïß«pJ"¢?"ѧ!I€?p*Gå¼nÆ?"ѧ!I€?ïšgå—sú?'w >‡?‰f§áqO?'w >‡?ïÿº†ŠYq>öûô1`Ùð?^l›¹¦>öûô1`Ùð?ïùÏÓxž³?I³·Ü\?HÀ³ƒ*ˆ?I³·Ü\?ï>
¶"¢}?°ê0Ê®I?˜>©?LK?°ê0Ê®I?ï¿…³Õý?•®Ô93Ń?œHI…@W?•®Ô93Ń?ïúÀn"P?Dbò˜U?DþGžáƒ·?Dbò˜UAGN3FGL J0148.3+5200@`xwß (À#Ä9 1xÀ9¸þ›{ñéÀ;%îÇÉ?փՁò"@cFçp?üRóÀ+©§?ïýìH#k{¿¿Î'¢À¿ã¢+e"]g?¥©yámmÂAGNbcu@´1‹àÞ҉PowerLawGB6 J0148+5202?ïâs	·ä³?¬ç™úäùo?mŒö%¿4ç?¬ç™úäùo?ﲖ
Úx?'˜å	q¨?ƒZ|'Bt?'˜å	q¨?ï¶ÿþÓZ0?'¼ÉQq§'?'@SÀz?'¼ÉQq§'?ïùó‹[?8à/i	R?I¼2K…Ó'?8à/i	R?ï÷´͇?Q®š¬of?Qö—ŠlsO?Q®š¬of?î$K
ðY?¸Ø˃?§-»LEz?¸Ø˃?ï[2ì™úE?É—Í·dx?"™¢qè!R?É—Í·dx?ïÖ;4xF|?r2RO½‰?tâe±þÉÙ?r2RO½‰AGN3FGL J0148.6+0128@bÝ"ß°Õ ÀM †¿¢AßÀ9ÀX·Q:…À;ŸŽ'å".¿ÙXim×ÉÖ@†öA»6L@*@\fˆ¿Ú³ßæ…·¿æ—Oß³§¿Üvpd_¯¿Â•Òÿ[AGNbll@£MIº^PowerLawPMN J0148+0129?ïÿ£¦Z>²?Ê&¦¯?oºÏ:?Ê&¦¯?ïÍƧG?'¿Q™b­˜?y¬"êø<?'¿Q™b­˜?ïñÔ5CP.?cªì%KIÆ?\W•/(÷?cªì%KIÆ?ïÿ~PpŽf>þ¨"BŠA?5ùWÃ>þ¨"BŠA?ïÿ¦·Ëo?eŽ»áf?R^[&Ô?eŽ»áf?ï]ºhF:w?«Y߻ھ?"H²÷8±!?«Y߻ھ?ïåóã¤f?s®/Ò¥Y¹?jóÜ:&?s®/Ò¥Y¹?ïü†Fç¬2?1ÄiØûa€?;ÍÇ«WÈ(?1ÄiØûa€AGN3FGL J0150.5-5447@qÚ®_ú;›ÀN(}?Æ¿mÀ:ÎakTâ°À<*'ë"z¿þøYÐÖÇ¢@CpcÀCÒ@ò -1'¿íïÔ.ž"¿Ý¥Zõfkf?aBàÖl«¿è2£Ý¯AGNbcu@¡=ó¶E¢PowerLawPMN J0150-5450?ρ™.?¢¶À*ƒàj?‹"Œ™´ƒ?¢¶À*ƒàj?ïÙãn#ôý?‡Ÿ;'rûí?sHîµmž?‡Ÿ;'rûí?îמ¿ô!P? ÖºÂvA,?¢†ÿ
? ÖºÂvA,?ïÿøâe¡>ÅaÍ¿¥¿>ÌuæÜ+v>ÅaÍ¿¥¿?ïlÏÃf
?¢âÓ™¤ô?'fŠ§¨?¢âÓ™¤ô?ï15
\h?²€Rç&Áë?™ÙN3«?²€Rç&Áë?íÓ¥Gçd?¬¡†¨ç´?±bÕÂ|­I?¬¡†¨ç´?ïÿ¯ñ}câ?'¼äÓðŒ?¨W˜kA?'¼äÓðŒAGN3FGL J0151.0-3609@oƒÿŸ‡ð$ÀR†À
¡©À:mtòd/À<gpQ¡³Àæl¿@+-']¶@¬]·ñ¿çųT
{¿å5m:ž•
¿åžçsŽr¿Ö"½.t1«AGNbcu@‰TWsüPPowerLawPMN J0151-3605?ïþÁ¥ëü,?&=‡Bì!?#å¡×øÏ
?&=‡Bì!?ïàäÛ¦O?'Ï/$F5?o$'xç?'Ï/$F5?ﳕÊ	×x?z‰jlÆU?ƒ…F?z‰jlÆU?ïÿÿ«¶•>"qIÊÍã>…
ÔÎ=>"qIÊÍã?ïýÄ r?§?7¼Žfù5?1Úþíüî?7¼Žfù5?ï'bSb?"öˆªUuö?{§Z[‡?"öˆªUuö?ï!›†.?",aX6?œÉžJ?",aX6?ïÿí*æ2¤>ì8Ø­£†ú>âÔò™ü˜>ì8Ø­£†úAGN3FGL J0151.0+0537@bœ] l‡ÀKK¹ëÀ:o¢äßÀ;Ӓºǿޔ®tl}@
w¼'&á@@ߜÿªšž¿ë<TÞÕ¿âA¾¦:ß¿ßlsñTl¿à÷ŒŽ™5qAGNbcu@"m\ú¬ÚPowerLawPMN J0151+0540?ïÿ÷þ:?§¼5>‹?¼ObðZ?§¼5>‹?ïÝòìòB?€]ÄG¶¯?q‰nï›?€]ÄG¶¯?ïÎZÚ¨=Ý?vªxB°¤?xҒ¼_13?vªxB°¤?ïü+/aJ%?)Î5Q"y?>¦ƒÙV?)Î5Q"y?ïý½èÙGÚ?4¢ô'l_æ?2¸Ê Ï?4¢ô'l_æ?ï`Å AO<?¨zX''ˆ@?"ç[ùæ?¨zX''ˆ@?ïT»fe?'´¢RˆŠ"?•h"8í·r?'´¢RˆŠ"?ïÔÞ/h¬?h©²ÉôÞÂ?uÀhû–?h©²ÉôÞÂAGN3FGL J0151.6+2205@aœ~`Ï6ÀCU˟¦#À9½#nšÀ;º£ø'Ä?áÄDã‰Ò§@š§_Tú-@;[áF׿æÝÓG7p¿çݶÂs¿æœÛàæà¿ïÿ}¿|AGNfsrq@|Ú¹õY³ÐPowerLawPKS 0149+21?ïúŠ	P-6?G¹ û©«?E×Úί̷?G¹ û©«?ï'(*Û:?ÆLZ?ŸO?|6w=y?ÆLZ?ŸO?ïvRBJ°Ü?zT¹¹ÌI?'5·®ސ?zT¹¹ÌI?í¿8.ðƒ`?‹ã<6"b?²>‰Å¿|?‹ã<6"b?ïîÌ`;h?dÇËo gˆ?a3ŸöE89?dÇËo gˆ?ë{¬}å?Áðü'fð?‰NÀl?Áðü'fð?îČøT¸?™7:w÷½¤?£·0}R9~?™7:w÷½¤?Ẏ¤?±Ží®™°ì?Ýø‹ôâ·è?±Ží®™°ìAGN3FGL J0152.2+3707@a
¢À8+À~à±À:>'d@ò9À;ârÚ/­¿Â©—âùùš@&¶£Ã@@vÀP½ˆ¿Þr²™3±ø¿ä®K×¼6t¿åˆMD+~¿å–IÕ$ùÎAGNbcu@Ž+Ý/Ÿ¾PowerLawB2 0149+37?ïþ´P
?;øâðS?.T½»üf"?;øâðS?ïËÇzc¯Ž?ŠҔÂ,P?zB¼JA?ŠҔÂ,P?ïµ}1Gåa?{†0"‹ú?' ³¹gÄ?{†0"‹ú?ïíû9Wö?E˜ôS§?bÆyN³?E˜ôS§?ïði¶–ÄA?i±O›"7€?_,'©<.A?i±O›"7€?î÷Á$…?±öˆ¹]Àa? ƒîžš¨?±öˆ¹]Àa?îŽ	ôܜŠ? Œ>á=ýO?§`³b? Œ>á=ýO?ïrl6½Š?Š·÷3Åئ?ñ²p'HÎ?Š·÷3ÅئAGN3FGL J0152.6+0148@co€UûµÀLÃ)ßÍZ'À9qè
šó6À;rÔ#&v?'¤ŠŠô?v@'˜ª†Pç?þ/žÉ.]¿ã}ûüþ¿ÎU²;Hwà¿æ1ð\7Ó¿—TŒQæ_AGNbll@ª*²a|ÚPowerLawPMN J0152+0146?ïü®¯ç?7/xþ 4•?;—'z¤o?7/xþ 4•?ïÊT»ªKÕ?'Öd3öT?zÕ¢
MqÖ?'Öd3öT?éñ†ý?"Ð9óÿ‡-?‰˜…íË?"Ð9óÿ‡-?ïû^&·5?2^êÒÉ?B‡ó	Tu?2^êÒÉ?ïí
Üõ0f?c ʍpÙ?bõ"ès'•?c ʍpÙ?ïJýâ[?®›`cÛH?– \¥t"¥?®›`cÛH?îò — ×7?—}·´äX? Õöƒ^ח?—}·´äX?ïÊAšT)£?t¹›%åŠ?zß2֛Œ?t¹›%åŠAGN3FGL J0152.8+7517@_¸Ôýó¶F@)ÈÒÀ+ԚÀ:–›¸WËÀ;±"Pª<?ï¤ãŠå‡ë@1­@˜?üS ?ïD¹®j"§?£«ÁlúÞ¿Òò-¬-}¿ÛZâÃÈÛëAGNbll@¹$Ñ·PowerLaw1RXS J015308.4+751756?ïûöB^k¾?=—hU l?@&ö_Õj?=—hU l?ïOH-§iL?¤Fç5§ÙX?–úLʤx?¤Fç5§ÙX?ï·-³íWÝ?yÊxÿ?'4'ôÛÔè?yÊxÿ?îå)Ð]ûß?kÅwKA™?¡­bùD[?kÅwKA™?ïø:ò¢ÒÜ?N'‡öâX?O4Üùy?N'‡öâX?ì¦åGÆ?ñe-+\?ºÈÕÇGQÎ?ñe-+\?ïJÎA/ää?"æT¿<Cè?–¦7ØK•‡?"æT¿<Cè?ì¾k‡ÚÌ·?£Œ}ãkÛ×?º£Á)šG?£Œ}ãkÛ×AGN3FGL J0153.4+7114@_ûÞ¨—c@!òU¿û?À:Fó½Ò^À;¢nfåè'À›	º"å%@ÎkéG'?ù~àZÉ$?ÙhS.-î¿åVüæ¿Í$Àdð¬¿Ð¡}ÇñØAGNbcu@Ëò²° ĜPowerLawTXS 0149+710?ïÿñ2»G?Äí¥Ê5?aÔH{?Äí¥Ê5?ïΦ–#º½?‹ûä7X¤	?x¬µ
ÿY‡?‹ûä7X¤	?ïÞÓIò?l_l?ÏéÚ?pö–>*;?l_l?ÏéÚ?ïÿýÝw%7>²ó½ÿ=>±ýåq(>²ó½ÿ=?ïþuD‹ÜS?3,%Éý]c?(«»ˌƒ?3,%Éý]c?îÿk7(É?²ÈÌɛ	É? 	LŠGr?²ÈÌɛ	É?ïÖ,F"?w"ü`¶?téøç½Õí?w"ü`¶?ïÿßPTx >ö9–43a>ðW¶A«Ät>ö9–43aAGN3FGL J0154.0+0824@b‡…À3aVÀI® ö½À8)+rt'À;
ú滋\?ò…­¶Üöf@¯í|Å£c?ýÀ(~ú1	¿Ç'ދ'A¿ÞF²ZÊ¿Ó=ЊòaÝ¿á>qðˆ=ÒAGNbll@¡U:û~'PowerLawGB6 J0154+0823?ïê¤7#Ð?dXT¹@'?eÿ["¢ =?dXT¹@'?ïŠI\ÀJ]?Œ£Ñ‡ÅÒ?m¨átŒ?Œ£Ñ‡ÅÒ?﨤ëÌ@?€ï÷ò±ã?…ÖŽÐ?€ï÷ò±ã?î¼Fº?†orãÿÂ?®";"'gõ?†orãÿÂ?ïю¨ÿ?uÐzMgÚ?w8þMŸ,m?uÐzMgÚ?íUÙ"Æ~?·×6TŸ?µQ6ëñͅ?·×6TŸ?îûÙì´¸s?™d-ÜD*? Ba8ÿûÎ?™d-ÜD*?êDS¾C?§Ì¯}}ü}?Æó?§Ì¯}}ü}AGN3FGL J0154.9+4433@`Õø@À0Ý¿Sg†À:_`¸§|À;ÒËÖ,Çß¿÷1ϨÊ9@f.fš¾³@w€ KÏâ¿ÞzùWf¼¿âÕ
Ý}
¿è"õïʗ'¿¸b
CVÅAGNbll@˜ÑÖ8†YKPowerLawGB6 J0154+4433?ïÿ‰¼$´?!S™F¼?
ºÅÀ¨¾'?!S™F¼?ïÑlñ½>‡?ˆï'¯`D'?wI‡$ l™?ˆï'¯`D'?ïÑÉf:òo?m™Ãwï|?wLîå`J?m™Ãwï|?ïÿüµ¦H1>³™ðé¡M>ºS7{èSÛ>³™ðé¡M?ïý\°¾`?=Ÿ!_õ?5'l«¥7?=Ÿ!_õ?ïÖN^eo?±'Ouω?Ÿ%69Z¼%?±'Ouω?ïmÅbAµú?HË©iÏ?'GS°êÁ?HË©iÏ?ïÿ¾õ|L	?}"Œ´†‹?B™rЙ?}"Œ´†‹AGN3FGL J0156.3+3913@a
Ô2TçÀ5î¬_nû`À9ƒL8½¶¯À;Ë+/X³À¸ûh¾@(³Ä"t@öA?»VÙ¿åŠXµ	ð¿è_Pé/6­¿à¯öäV	¿ïÿë‹åãAGNbcu@"PVOv`PowerLawMG4 J015630+3913?ïÿ!Ä©?¥Ðu#Ô÷?œÃÁr'û?¥Ðu#Ô÷?ï×]Û³M?…®] c?tQ8gé?…®] c?ﯺ=†¦Ö?yÃÂ/5‡×?"p¢uÒg?yÃÂ/5‡×?ïÿÿáïk*>xîpV°>n0©OI	>xîpV°?ïÿº¬¨ƒÜ?~#¶9¸?TÚf5ç?~#¶9¸?ïG'°hµn?«T"
ÂúÝ?—
©ì
Y?«T"
ÂúÝ?ïÎPWÜ4õ?}L5Q?x×Ôf%³?}L5Q?ïÿü±ZÅ7>Ä[ۀ¸Õ>ºv•	º˜>Ä[ۀ¸ÕAGN3FGL J0156.9-4742@q6`ÀiçûÀPp×?íUÙÀ:õ©ŽÚ"÷À<&¬k-v¿ö¹Ô,g'@†Q
^¨­@¥ßx "?ü­–‰¿ïiŒFR}Y?ä(_ÂÞ6'¿¢·JüÊã¶AGNbcu@¬KK]ÌcñPowerLaw2MASS J01564603-4744174?ïã=ì8'±?¬Ü;eíÖÄ?lÂœÓ'Š?¬Ü;eíÖÄ?ïØÇÚþ'?‹fs	^ŽÜ?sœ|Ò·?‹fs	^ŽÜ?ï"Ý|"È?‡`1ˆ>¶?‹?¤Jiß?‡`1ˆ>¶?ïÿü×xï¢>²TŠ,ôÔ>¹Bá½-›>²TŠ,ôÔ?ïø«xûO¨?`¦™™†Ô?MRðN"?`¦™™†Ô?ïD5àË>?°
äe·î-?—yCñnA?°
äe·î-?ï*†®QÙß?•=©]ûÁ?š¯*>[Ê?•=©]ûÁ?ïÿöëâÅ:>֚z»+Èè>Ò'×¢'þÑ>֚z»+ÈèAGN3FGL J0157.0-5301@q¢ß?–ÀN°ŸõÔ-À9ž´À;(Âz?ò¦Ì,¾Ïß@Œ,ºÉ1?ý*
h¦?ÛM{'ƒ·¿¾x9cN¿Ì5¹åg¿æ WÊ}AGNbll@¦Û$Ý/PowerLaw1RXS J015658.6-530208?ïÞw²>+4?p¾ó!Hš¼?pÄ&é)v?p¾ó!Hš¼?ï];}b4?"kÀ›Ð¦W?"XXàéP?"kÀ›Ð¦W?ïNë)ç@?—ÿ¡Ë?–"Ÿœzåó?—ÿ¡Ë?í±O†Ù?'	Ø6†{?²w…"¥ö?'	Ø6†{?ïs;ljõj?•‹˜
7?'˜‡	™è¼?•‹˜
7?ì¦à¶Ûì?À'½™Ëe?ºÈúI Ÿ!?À'½™Ëe?íú3óÖ¶?¢{Qd^"Ú?°.`a½ÕÑ?¢{Qd^"Ú?êe³šîû˜?­4"3Y]?Æi1"DŸ?­4"3Y]AGN3FGL J0157.9-4615@q
?ÐÐhÀP²uÀjÀ9Áj©ÂÉÀ;çl¸ÿ?ðÎeä¶@H'"Í.Ç@˜[À6ã¿ÞôË·"ž¿çœû7昝¿æèf">®¿ïÿëÆj»"AGNfsrq@"´*͞ƒäPowerLawPMN J0157-4614?ì´Pb º?Ñ0WoÂI€?º]|îú/m?Ñ0WoÂI€?î­
¨áœN?¦/P+Æt?¥/UoR†%?¦/P+Æt?îÆqP™º?•sðÓíFx?£˜ïAçV?•sðÓíFx?ë•ü®¼Ág?šuÐÑ9$+?Á¨
Eúd?šuÐÑ9$+?ï|"\qM©?¡®S" Û?m"p|ì?¡®S" Û?æU]¶£ô?ÍŨøÿ}?ÓUE֒¸?ÍŨøÿ}?ë	ܬW¦?±‡±,
ß}?Ã؍N¡gˆ?±‡±,
ß}?ÛñôYX¶Ð?µÊI²‡?âÓS¤˜?µÊI²‡MIXED3FGL J0158.6-3931@p,Î?þó'ÀQÔÀ_×,À9XŠÙã5ÅÀ;Ã¯Ù`?ÞÖæü£Õ@ë«/™Ì@.HÿxE·?q×U¼Ê÷
¿ávþOž¿âÅ
¬N¿Ù»+ÅUµAGNbll@˜ß87´¢4PowerLawPMN J0158-3932?ïþ8Ý?*ܐü?,~yŒÚ÷?*ܐü?ïÈæßÙ«?'¨Ì+Vå?{ŒºÚ?'¨Ì+Vå?ïå7åQm?eô¢Èýp?jÈüíS»v?eô¢Èýp?ïà[üÄÐï?Rxäoº"Õ?o¤`JÙ?Rxäoº"Õ?ïþ&AïIá?)"¬"ýu?-›ßt9å?)"¬"ýu?ïA¹9XLƒ?«ŠMSrý?—ÈØÓ>¡"?«ŠMSrý?ï±|Ì{»…?†å¾Éˆ?ƒ ÌÔZê?†å¾Éˆ?ï9±ñ˜øÏ?"}ØÓHð?˜ÉÁÒP%?"}ØÓHðAGN3FGL J0159.4+1046@b–¯ÀL‹ÊÀHT(?º*3À9MPíX]À;€¯°î¿Ð	'û%áÍ@Ê#EÕLM@èHÞ½¿æ=ô$™V¿á©'¯èˆ¿åãtó·¿ÇÃ\ôÖ3ÜAGNbll@œ
Ú¹õZPowerLawRX J0159.5+1047?ïþUCån@?&ª˜*œ©&?*«¿Y'}Ê?&ª˜*œ©&?ïܑÝ)3?I*®æó?q·uu>šÁ?I*®æó?ïÜÚ5wð?pJŬ`0m?q'åI<?pJŬ`0m?ïþe;¡ŸU?H%Lˆ?)¬B¸g2:?H%Lˆ?ïý:#£"e?5é'°?6.ã4 '"?5é'°?ï;Kfþ?±'f²W?˜œ6'hpø?±'f²W?ï²>ÊÎ{?"_>m?F?ƒpMtÄÏ[?"_>m?F?ïîЇ\$?UûxÏÿ!?a/y@C¢?UûxÏÿ!AGN3FGL J0159.8-2741@k`–óEÀR´›€#¦ÎÀ9þ¹=£ÏÀ;ضXí ?î!J˜]7@Â5'ÿùJ@JIÀ4¿ÓdTªô'@¿Ó§¨Ì£˜\¿á-=…œŒ"¿é~"لý<AGNbll@šzÇË)PowerLawPMN J0159-2739?ïãaÍ/c?q™;ˆëÄ-?lž2Ïít?q™;ˆëÄ-?ï©æâ]éÑ?Š­¬Å4?…†G^6·º?Š­¬Å4?î»ÿ…0Öâ?›¢ˆZËá<?¤@­Îx×?›¢ˆZËá<?ît‹Ýeá?'ðäˆC?¨·B'ë÷ø?'ðäˆC?_P{ ?˜ÈZ$?¨/PÓí?˜ÈZ$?í|²áœÆ'?·ßëô–|?´hóÎÄ?·ßëô–|?ê7ߢ3é^?¶Š·œ)ó?Ç w0Zˆ?¶Š·œ)ó?é<"¬l?§%Rb
?Ë«ñ­NO?§%Rb
AGN3FGL J0200.9-6635@rGÆŸ¸ÀHñ7À:/œÔ·|ÙÀ;ñò¤ÍªB¿ï)÷é00@î#Ž¥u@¥ Z¨î¿ãµ¹óA‰¿äÔÂâ4µa¿ç+À"‡b¿Þ(>Ã4G°AGNbcu@"nËûµPowerLawPMN J0201-6638?ïþŒÑ#¸?+ã96‰ª:?'?všóÓ?+ã96‰ª:?ïÔȃ´Lp?‹I. ÿx?u›¾F&õ?‹I. ÿx?ïÈß\=åá?€úþv°'?{QÊ_£–?€úþv°'?ïÿÀ‡¢\>ñb¡CqÂ>ÿ¼—)Ìü>ñb¡CqÂ?ïþž[uF©?$FTU–zn?&Lj["?$FTU–zn?ï< ½"?±`Ô
*Wd?˜{ÿNo?±`Ô
*Wd?ï®ùŠšù?ƒiû1GÁ?"APª´Á?ƒiû1GÁ?ïûßto=¥?9ÃöÅ7—¥?@'.uC_?9ÃöÅ7—¥AGN3FGL J0202.3+0851@bݍ`¦3ÀI/ÿ¢/À:€\GÿsÀ;ÕiŠÞô?ï+Í+þqÇ@
=`'@as\f³?ïÿ—›UÊ¿àZ¦íÈ£{¿à¯€`¸}¿éo~ýOæ6AGNfsrq@¢o¹õY´PowerLawTXS 0159+085?ïà€q»•S?:®\¶?oŽ(íÍ?:®\¶?î
–'h­?®Ô´šùVs?¯&Ÿ‰u,?®Ô´šùVs?íÙó1<?¢Lùæ‡õ2?±0c–,›¢?¢Lùæ‡õ2?ëQèß
R_? ]ë5ÌX?¸\ƒÊ¶ƒ? ]ë5ÌX?ï"`˜2^?ÑYВ?‹'ÿóh?ÑYВ?çZJ%Š?ɂ",¥¥?ÑKËk´ë?ɂ",¥¥?ç¼CT_ö?¼*[.‹?ЇyW@ý?¼*[.‹?ஔN<_=?µ
N­n*?Þ¢×c‡A†?µ
N­n*AGN3FGL J0202.5+4206@aԀuÀ2Öÿ_ÇôÀ9臢 PØÀ;ӗù†i;Àת´*8@z*ßQ´©@4JŸá\Q¿æñO:þ¿æêPé|…ã¿Þ#q_Ïڅ¿åíTW°@AGNbll@'¶•fÏAòPowerLawB3 0159+418?ïÿzÊÒ!?sü"ÂÃ?¼âm"K`?sü"ÂÃ?ïÒÍïÙä…?‡;§C¡!?v™"Ûñ‡?‡;§C¡!?ïîxciþ?k6·ïgx×?a‡œ¶–iã?k6·ïgx×?ïÿÿՖR›>uNõdÆ>uVÜ5é6>uNõdÆ?ïþîÏùIz?"2žo|?!\ÂhÅ?"2žo|?ï3B!¸Œy?ª´¹àªÝá?™—»ÎÚÚ?ª´¹àªÝá?ïޞ¢S7Ç?t•]$ÁPþ?p°®ö°p€?t•]$ÁPþ?ïÿùŸé"Ú>Ò5tT©N>ɁiŒêí >Ò5tT©NAGN3FGL J0203.1-0227@drä¼®ÀMøK¹ëÀ:hØÿ
6»À;ðL'8¿ö+?(´Õ	@ُ'Î@€Ÿ¨Qm¿ãÝêŸÛÜ¿ãÂ73&¿ãJ<ɦ¿íǔdâ"AGNbcu@'ëWsüPPowerLawRX J0202.9-0223?ï×omÿ•€?päê1Uó0?tHHö–XG?päê1Uó0?ïÖÅ⟃?ŒÞÆf¯¡?t?þâ
"?ŒÞÆf¯¡?eÆó?'u0W"ð?¤$™¥H?'u0W"ð?ïÿp·^aÆ?*ô˜eÎS?é*òȋ?*ô˜eÎS?ï¼2Àòy?|gµ²?€óOȉ)?|gµ²?ïbrÃccõ?ªGô6Mbí?"±§šr¹Y?ªGô6Mbí?í¡n«`Á?¦s€…jp^?²ô‰éÉö?¦s€…jp^?ïô•Š…r?Q­ê†¶…ë?VÔëyÀH?Q­ê†¶…ëAGN3FGL J0203.6+3043@a™Wÿ›V2À=¢ê šª;À8Ký¥²¬À;3˜ÿ?æ ?÷ÃkQݘL@†Êò9¼?ÿ?Ü+zÝ¿Ô\ãÐõPz¿ä+y@nì¿äAÜÕiº•¿æ{¬F‰@AGNbll@†:Ø_ö"LogParabolaNVSS J020344+304238?ïþCÜðþ¨?.Cß¼µ?+Â4TZ?.Cß¼µ?ïÅ'ÀŸ~?]§H¡?}l"ā?]§H¡?ï9­Oâ~?'$.Úõ3½?˜ÊV~I?'$.Úõ3½?ïþIò5·?Êüðœ?+cÁd<Ïd?Êüðœ?ïüž0Ø ?@sÉ6Nu?;z?@sÉ6Nu?ïÖä9K?²ùÃð*+?že#xޖ¬?²ùÃð*+?ï"µ¶tŠ…?–Û‰¯êßt?›©I8MçN?–Û‰¯êßt?ïþ}âÝ?"Ýf[ú€ö?(!ۋúüë?"Ýf[ú€öAGN3FGL J0204.0+7234@`î¿eÛý@$ô "AÀ9-¯d9ÖÀ;aâÔvz¿ºýŠ*¡ûN@,F|ç_@ÅÈÿ¿F¿ÙnQÂ?€¿è‹ÌŒ¢å¿Ü©ÁÕwì ¿âê%Š(8AGNbll@š	ÆYJôñPowerLawS5 0159+723?ïþdžKk?. ²Y-i­?/I³¨ŽÍ?. ²Y-i­?ïϸÖ[ýé?'š†{,Æ?x#"è®wq?'š†{,Æ?ïÒ]âM+q?vWI¤Ô?vÑÑÛ#°?vWI¤Ô?ïó2¬rÎ?A{°V>A?Yš§1ñã\?A{°V>A?ïûZXæ÷?AUùíF¬
?CŠ–¡ã":?AUùíF¬
?î¶ÇO4p ?¶ì#N­šÕ?¤"‹('ü?¶ì#N­šÕ?ï£A¥´&…?Š‰A¦¡;?‡/– ´Î¦?Š‰A¦¡;?Ñê»B?|ØÖ°ý>ª?Q‹Œ0g‹?|ØÖ°ý>ªAGN3FGL J0204.2+2420@aí" ³Ô®ÀAΓ [TºÀ:ÑÊbAÀ;șÌÅ@¿Ê/'Šxá¶@
Óú=ž?ü­ŠÒS?ÕÛç·èË¿Ú."f\‰¿âÛ@°…€?´ïA8P÷AGNbcu@´»dZ¬PowerLawB2 0201+24?ïÿ‡e˝?'Z××â?/Šƒ›‰?'Z××â?ïÐw°Õd:?‹5r¹ÂH?wÄ'²*ší?‹5r¹ÂH?ïØÎËO—?h'SÂ"c}?s˜ó2ex˜?h'SÂ"c}?ïþ[á/ãÑ?WF'%]æ?*Aê\vZ4?WF'%]æ?ïýòîç?+äЇҎi?0h¼aL?+äЇҎi?ï@îÛsn?°"¯Í±þ?—â$æÄC?°"¯Í±þ?ï¦lzbÙ?ƒNTí¯Ô?†{dèFÃ?ƒNTí¯Ô?ïï&*®vÃ?\´3Ø²U?`ÙÕïU~?\´3Ø²UAGN3FGL J0204.8+3212@aü–þµÀ<%»À5ÖÀ9F	ç	ŽõÀ;åŒ·3?ÞÜ~¸@!↝h†@Ž—?w9G¿èð+Ña~m¿èz—U'пïÿì%úÝÏ?ïùqæ¢5õAGNfsrq@sóºKâPowerLawB2 0202+31?ï]kÚTÜ?Á¹k"f	R?"^r'ý–†?Á¹k"f	R?ïÄq}µ|=?'ú;2¬?}ÇA	Ŧ?'ú;2¬?ï­‰·×Ñ?ƒ'íN9<?"º]ŸÈ{½?ƒ'íN9<?ïÿUwDžÚ?ôԚóÍÖ?Q7¢í?ôԚóÍÖ?ïû
µ•#?P¡®:?CÉÀaF%?P¡®:?ï*^¶;?®6ó‹lI?š´=sxԚ?®6ó‹lI?ï=.çÀ³?'qìÆ+6Ô?˜Z<w…¡?'qìÆ+6Ô?ï5OÝ?p#85ð ?`uiš•›r?p#85ð AGN3FGL J0205.0+1510@b€ºÃ.¾ÀF	՟Ú%{À9M­Ûoý¿À;¦G'ܾ¿ñv8;/ÖÝ@± üÏÊ@= v­†¿æ•'¢)`¿æzò@"‡Ë¿è*…ŽŽ'n¿æt=IaÕAGNbcu@ƒ	¡ÊÀƒPowerLaw4C +15.05?ïÿÖë‡>ð¡\+
®>ôý˜Ó¹ñà>ð¡\+
®?ïÎœ'WL?'ŸUɟÁˆ?xò±þâ>?'ŸUɟÁˆ?ïä§ù¼?X©Á©ú?kXLÕ?X©Á©ú?ïÿӐ>Ï>靝ªŽá>ö7ÇOå,6>靝ªŽá?ïÿ²‡sž«?â×tñ?^x®¸{?â×tñ?ïVzâŽ÷?­G¢O!†?•0£©w0?­G¢O!†?ï×ÅWáú?qÀ8¶ËÆ?tuÇ~Ü?qÀ8¶ËÆ?ïý|Ó\?0:%ú‹{/?4i@9΄?0:%ú‹{/AGN3FGL J0205.2-1700@gB¨€QÉ÷ÀQ‰ÿ`2o¿À8ºyà–®-À;¹C'&?ëÉîóµ'>@F‡7¯D@c¿Âù¿æ»§[¬¬¤¿éËÄOr&¿ìÁ®Û¿ïþ%Õ|ž·AGNfsrq@u0O‹YPowerLawPKS 0202-17?ïýV³ý?0Ý-PÎ2?7Jw.ޕ?0Ý-PÎ2?ïÕfûé?Ž‹zݞr?uL·unm?Ž‹zݞr?ïoçAÿ:?"°zMýM™?'¹9"÷?"°zMýM™?ïéú½ÿ] ?NéØ¥è?fBB›_/?NéØ¥è?ïüϾ¦×?98ôzÈv?9'·šÛ	?98ôzÈv?ï*Õ(íÎ?°ît%6ˆb?š¥Zó	°*?°ît%6ˆb?ï]Tª"Öò?:‡v'"©?"Uj¦Î¾?:‡v'"©?ï¤P±@Å?zoøI¹Û?†ëÓ¯1^Ü?zoøI¹ÛAGN3FGL J0205.5+6448@`VþKZ@£ÿywÀ7¡Û§[#<À;»·Ñ"?ùhÎÆ!7@ú˜Ê¼§;@¦Åæ(¾e¿àƒQé3$¿äŒ–EYÚ¿çè-µè&<¿í
9äI¸}PSRPSR@Ü\ú¬ÙèPLExpCutoffPSR J0205+6449?°exó?²Ïœr´½?íý³[Ùçà?²Ïœr´½?ª,:³_\?Á"‰"(?î]?ÌÐK?Á"‰"(?Þ>
N>Ÿ?´ƒ·|š­?à÷`ùXà±?´ƒ·|š­?¡}I<@q?Š_†"nië?îè+l.@I?Š_†"nië?lL´?3…â?p€·Û,È?ïã³KÏêÂ?p€·Û,È?‹`A¤´+ ?¦¼Ö>n'?ï'~ù–j¡?¦¼Ö>n'?ÀEªj]}?¬þDvš|?ëî•eh º?¬þDvš|?e)%yÊcì?[äGšJÒã?ïêÖÚ[št?[äGšJÒãPSR3FGL J0206.4-1150@eóWŸ#FVÀP¬Å@'HÀ9Z&d׍À;ÄAvÂÔü?²dŽPvv:@Gµpå›P@¦½M¿ãºÞì<²¿åRÙr2ދ¿ß¸ôäÕ}¿ëM‹,T­èAGNfsrq@ˆ'Šû"ŠPowerLawPMN J0206-1150?ïÿ#›ª?)´z›"?œ,ÈNä'?)´z›"?ïÙz¤OÄÓ?‹¶YK~a8?sB­ÐŽr|?‹¶YK~a8?ïÍäTÜXä?s5$‰&!?y
Ց#¡Ã?s5$‰&!?ïÿ[)òAÑ?›f¨ÐM?šÆúäøÂ?›f¨ÐM?ïÿ
PÂ݂?!Q=å×î‰?Uâ¾ÞC?!Q=å×î‰?ïFb§ýz?°D¢
EB?—3«&ˆ±?°D¢
EB?ﶜÚ@Ó°?….ýy7¼?'XÉbdš#?….ýy7¼?ïþeÔxÆ?&
Nñ7öX?.	 1ðR…?&
Nñ7öXAGN3FGL J0207.9-3846@o»'_ét£ÀQT_Ó¥.À:,x'¸ÔÈÀ;ü6'cDs¿ÔýÃw"@÷Îú¤vl@Zk@•ÇR¿ã[c$VeV¿é&çx¨:û¿ã¥¯½ƒ¿ì	i4àeAGNbcu@'âwškP±PowerLawPKS 0205-391?ïýëªL^?0"v6Ö2¢?0¢­Ô	
7?0"v6Ö2¢?ïÚòûñ¹§?…"¸;ù³é?r†ñ%¬k?…"¸;ù³é?ï—xSñE?GÛ&zê·?Š!ë+Š¡?GÛ&zê·?ïò\CLÛÑ?E*
%,Cî?[GyÐ~Ì?E*
%,Cî?ïÿ~;'ž?!%á<­y?P4Ozû6?!%á<­y?ï/ìÌòa‡?°Íù?€û;?šfa³Ï%?°Íù?€û;?ï°¤À"/L?ƒˆÁŒR5c?ƒÖÏÓ¼þí?ƒˆÁŒR5c?ïV/µá_?"H¡7ÕOÄ?•:	Hû‡Ð?"H¡7ÕOÄAGN3FGL J0208.0-6838@rMÀÓgÀGy¾Ÿã_¶À:	~(úË
À;â½µÔì¿ÝÌǗ6pˆ@ÞXºla@]HÀŽ%¿ãâú˜ž¿çZ|Oz£¿â"Œ c¿æKõBÑz AGNbll@ÿ¹¡vÝ­PowerLawPKS 0206-688?ï²âÝn'?´òZ¢yAS?ƒGy",ø??´òZ¢yAS?ïÑ;JȔô?ë8cAðp?wbZ®Cj#?ë8cAðp?ï½T†ý¥?~0ú}ö©?€ªÞs9ôÉ?~0ú}ö©?ïïRËKdÐ?LPiô?`­4¾:C?LPiô?ïùxåà?O¦rÍmÆ?JkºW{?O¦rÍmÆ?ï$a€w?°DnU,´?›sÏüP?°DnU,´?ïYë­§\j?ŽkïDúc'?"ŠI\¤Í?ŽkïDúc'?îé&+Q¬?'î?aŠw?¡n}Ÿ³:?'î?aŠwAGN3FGL J0208.6+3522@a‡?'æGÀ8á݀y7$À:v¦—®ÝÎÀ;¾Â±(,¿¶ÄY'À@
F¹q?ûG޻⚿ïÿæƒhf?ïü™¬l¥¿ÆFóƒN¿Ý|æì™×éAGNbll@¸¿£S÷ÎÙPowerLawMS 0205.7+3509?ïÿj®co?77»³Ù?'¨žóU…?77»³Ù?ïÑñ/VÒ?ˆóqàB ?w~]U×?ˆóqàB ?ïàZÉ­¼?f4G
M²K?o¥6–ü£?f4G
M²K?ïñýó$>=?EÄO_ך?\Ȧ¾?EÄO_ך?ïþÿÆ&ô?-(_"ÞAÖ?/@ýh¿"?-(_"ÞAÖ?îïòaÿH?²²Ë˜?¡ÙíV|?²²Ë˜?ïÓpÀvA?tlØ噫B?vyÇ­ƒOc?tlØ噫B?ïµ¾žô!?vÈy…ÄÑß?'[Ýk›?vÈy…ÄÑßAGN3FGL J0209.4-5229@qeˆ`VíÀN_JÞ™À8"Š¥àϹÀ;¤TÞ¿¸ýûh@ꨍþ0?üÊÈ`Ví?¯'®\¹Y¿á#}ë麿Ð*.QÌüH¿ÜàÏT!ÑrAGNbll@¦DÂ@·€4PowerLaw1RXS J020922.2-522920?ïÿŒ©,oÜ?
Sêé´[?Õ¼Ì2Ê?
Sêé´[?ï×VÙUœ??‰@y&
?tT"`àŒ"?‰@y&
?ïà-¦Ÿ*?m¤Ú{?oÒêM=¥?m¤Ú{?ïý¨)UK?"DE"«@?2¾³kg+,?"DE"«@?ïÿnLûÔ?ØPÖÊ5?=Ø©¦?ØPÖÊ5?ï0d"Ý¥Á?²"›z'B´?™ómk*â?²"›z'B´?ïêB߬+?rŸÙ—"'?e½ hrˆ?rŸÙ—"'?ï÷Rûáž|?D®oˆ.ÓI?QZ/—˜?D®oˆ.ÓIAGN3FGL J0209.5+4449@a&uûmÊÀ/Â\ÀË6ËÀ:BÖ?<VÀ;ÒØ|-x¿ä©gög¡@Ø j™&?ÿ'DÁ%#ѿ߃õK$¿éw";ueÌ¿Õ²«·1Æ¿Å͚xÍØLAGNbll@§ØÚu%FPowerLaw1RXS J020917.6+444951?ïÿ¨Œ{£å?ÉÅ&O4?ÜÖP'@Ö?ÉÅ&O4?ïÌÞ»•Jˆ?ŠÖ©äMC–?y¢,kÀ?ŠÖ©äMC–?ïî	r?X¡+òiÄá?aöé¸4I<?X¡+òiÄá?ïÿªÍ…>óš
"Ñ?LÄWc/M>óš
"Ñ?ïÿ‰þφï?^ڀrÕ±?
€<AGÿ?^ڀrÕ±?îúÑ(?³ÔûÍôȝ? ^_Ú»z?³ÔûÍôȝ?ïèŸP½²©?kº+$½ïÐ?g`¯€&O!?kº+$½ïÐ?ïüèv ˜§?3*N÷¼?8¼O^»Î?3*N÷¼AGN3FGL J0210.7-5101@qAÉ 'RTÀNâD?Êñ*À7²¢
¢À;5ʎ.+Œ?øêò4:o=@úJ´Y9@»zú;¿ât}ŸÔÆ¿ãÛb¥þ¤¿æéãC!¿èDUºœž‡AGNBCU@xôðØDÐLogParabolaPKS 0208-512?ïøˆEšz%?QÌ[°ÑSÐ?MÞ螳‹"?QÌ[°ÑSÐ?ïÓ(C'?Œ'܅*
?vvëôw7!?Œ'܅*
?ï(ÖoQ¶E?•Ð&å£Ý?šå2É7c?•Ð&å£Ý?ïþ-ÕÉÝ?¯8™ãt?-"¬§7Ø?¯8™ãt?ïó†Fb?VÒµ)mž?XóЪy|?VÒµ)mž?ï0¹!Z~ã?´®?™èÛÙ׍ ?´®?îqðq±aü?¡ÂïêŽGº?¨àøèY|:?¡ÂïêŽGº?ïþ5 Ywý?&'÷ë¥b?,­þW§J?&'÷ë¥bAGN3FGL J0211.2+1051@c}sÉÀG®ÀGƒLÀ7Ƨf
öÔÀ:ì)é•ö?øf)Kf†@4ïY¿Ž÷?ÿU¥`ÍX¿Û\™Õ9éí¿ä1øh1οà÷[s:¬œ¿æ.â톼ÙAGNBLL@"P´9XbLogParabolaMG1 J021114+1051?ïÿvQH¦?BB[A¬Ú?Ñ5Ðw?BB[A¬Ú?ï×1$e:?"M¨ˆ¬'Ç?tgm܁<­?"M¨ˆ¬'Ç?ﺍCŽ¹Û?€Çó¾ºû"?\¯jo.?€Çó¾ºû"?ïô¤Ò²À?@"tƒÿ¨?WÖ¶&`p'?@"tƒÿ¨?ïþ&~s?-Yá:,/E?-˜ÏèðÎ?-Yá:,/E?ï9"¬/üÐ?°c»oºõu?˜Ûª'Ïé?°c»oºõu?þÎ?i£‹§l?ŒP8Q«r?i£‹§l?ïñâ·UþK?R,ñµÅ`P?\:'ÌõªO?R,ñµÅ`PAGN3FGL J0211.2-0649@e3<`ŸÀOI¥ÒÀ:wò
ÎõœÀ;ò¼.ÿ?ÒIWMöÁ@ÿsì@Ë·À A¿Óì¿þC¿àÆۘäà6¿ÓYú6+Ný¿î‹o5~"VAGNbcu@œØÇâ'APowerLawNVSS J021116-064422?ïu#u"?¶—Gÿu?'['_ßÉ?¶—Gÿu?ï¸4W~Ç?†_RêÁQ?òê*o,?†_RêÁQ?뜪‡Al ?¨}Æe?ÁUâúO?¨}Æe?îÝlEÇF?†õ8è(?¢)>+£‹¥?†õ8è(?ï6KŠ±¹?˜'<eÿÖ?™=6—@ÎÒ?˜'<eÿÖ?í¿ýêã"?¶*ÔÅu²¸?²ª0æ^?¶*ÔÅu²¸?ìϋԒœƒ?¨RHEj͑?¹ƒ¡\´ög?¨RHEj͑?臮rn²e?º"ìN¥Ýþ?ÍáF6E6k?º"ìN¥ÝþAGN3FGL J0211.7+5402@`Ԙ€"åÖÀô'€—†À9¶^®@¦À;DDЩ*¿ü^øáӚ@
»Õtç·@‡¼à²^¿æyüàÎü¿é´¡¿¥>`¿ædŽŽ½ad¿çŒ
IYAGNbcu@";DЩ*PowerLawTXS 0207+538?ïúE/Må*?Q¸‹Þ?FëB™°¨B?Q¸‹Þ?ï¼î¼?'Ûä'Ï?€û}q$š?'Ûä'Ï?ï©InIc?{HÐÞ:AŸ?…­¤ŠÛ³?{HÐÞ:AŸ?ïÿÕÄ~Zà>ñf¥&\p>õ¨Tµq>ñf¥&\p?ïÞVô:'?s²£¥Ø]?pԅ"†4º?s²£¥Ø]?î|.sI½}?¸HþKŸæ?¨=Í÷Ý+?¸HþKŸæ?î¬æ™ì>œ?œ˜p^=Ì4?¥1–býA?œ˜p^=Ì4?ïúç±÷Ö³?C×$b*ÒÀ?Da7i"ž?C×$b*ÒÀAGN3FGL J0212.8-3504@nOЀ¶sÅÀQ¹¸!ïÀ:f°8AÀ;êTà,%"¿é#äV‰Ø@rå$ÝZ@ã矋öï¿Ë—pe~ñ¿è½VÃcË	¿Í'$[:¿ßdGKݽÐAGNbll@™
$Z¬PowerLawRBS 0292?ïÿ"M‡ûÀ?+½2VÅa?
ì ±Ëêê?+½2VÅa?ïØñ°d•?Š\?ÌÉ©?sÀ8ûÁy?Š\?ÌÉ©?ïç óÑ°?iq–àG¤?hbߌèS?iq–àG¤?ïÿŒC+	)>þë`èH®Ô?ï?¦íI>þë`èH®Ô?ïÿ¹¢è;­?bÕ6."?—Iz2÷à?bÕ6."?ïJ5œ€:?®X©¤Ô‹2?–¹Li‡?®X©¤Ô‹2?ïìs<ù¡?oV·5ýŽ?cŒÃ¥??oV·5ýŽ?ïýÓüJ?.›æþ#7Õ?7g£yIÏ?.›æþ#7ÕAGN3FGL J0213.0+2245@bN¶¿DNÀB,Ì?ß À9L=Ÿ¿™À;ƒ*¯ÖòÀ¿ø9§v@ò3ä‰@Éè <öÖ¿ØɄ\µQu¿â\û"+7ß¿æ'Y=çtÌ¿Õ$olZ­\AGNbll@˜E%F
¦LPowerLawMG3 J021252+2246?ïúOÞì–?G
PÆ)îæ?FÀ‡'€œ—?G
PÆ)îæ?ïÙ\×`=q?"êU-_Ý×?sQ"TÏ[?"êU-_Ý×?ï'k܋Ëj?‡ü˜¸
W?eî;1"?‡ü˜¸
W?ïÿߙX+:>涷—^\>ð3>`þÀ>>涷—^\?ïçp"jV?néí.\®?héˆŠQ?néí.\®?ï>rR>!Š?±á11í;?˜1µ½c8º?±á11í;?îˆ?'™]E?Ÿ…¾ïŠ)?§|
…ŽD³?Ÿ…¾ïŠ)?ïü¬ö›¿?;qÉêµ?:˜P¢£Ú?;qÉêµAGN3FGL J0213.1-2720@kJµa
ÜÓÀQöÛÖÀÀ:ØU½¡¶ŸÀ<†Ï'yë¿íòcއñb@òSDÀ@µ­S·ã¿Ë—$¹¿¿éª"‡Ð³%¿Ýç'/xú¤¿º)¸[â»AGNbcu@¡UeýŠÛPowerLawPMN J0212-2719?ï㾸%å‡?­ò½r?lAHÓé?­ò½r?ïÑp×>ÑÞ?&eŠí[?wG"z´Ñ?&eŠí[?ï¨M!×ý>?†Š¸DwŠ?…ì·ƒ!xš?†Š¸DwŠ?ïÿÄZÚ¹l>ðÝái\b>ýҁ†Õ¼°>ðÝái\b?ïüsä¤
?J6L` ڍ?<gÑ
st•?J6L` ڍ?ïU˜Jº
'?§âhõŸÅQ?•Lö¨¾O±?§âhõŸÅQ?ïO¡"z<?'åQÁìP?–ÜÊINx?'åQÁìP?ïüª¾2?5î%j‡ß?:ªÃÜOâ?5î%j‡ßAGN3FGL J0214.4+5143@`øÈS'^À""Vßà¥ÈÀ:'º'GmÀ;²B@p…?Ýóõ°›¾¸@ӈþ–É@Uü?V,2¿ì=b\I4°¿íeÈ9ü6X?ä)¡¢¾Ë¿âp6,·ÄAGNbll@«°Ø_ö"PowerLawTXS 0210+515?ïæc¦î—?¬Oךs?iœY©ÊØA?¬Oךs?ï½)•PV?†d®r?€µ»XD0z?†d®r?ïé¾m—Ú?re¯Óˆû×?fA'jOýã?re¯Óˆû×?ïòç
j̨?OB.œu??Z1å W?OB.œu??ïÿÞèXD?«X¶V2D?$!qð](?«X¶V2D?î*Ñ+p
?¹("†7Ñ£?­RíLnú|?¹("†7Ñ£?ïÐíüp¤?€Ò¨ Éí?w‰#ÅÏ?€Ò¨ Éí?ïçyo¸u?rèŽ+tË?h†çÁÁë?rèŽ+tËAGN3FGL J0214.7-5823@q»O?Ù3ãÀKØ'tÀ:MvÁ'}À;øшp¿¼ƒõÃf@ÿ/[bQ@O@…Z¿çs»
²›¿è'Í–ð¿âµpŸÐ?s¿Þ*x™Ä·ªAGNbcu@…èj_"ÊÕPowerLawPMN J0214-5822?ïÿo;Í
µ?GژèJ?ƒ'Ç©Y?GژèJ?ïÑéKý‰?ŠTð$ô3Í?wZ%4GÓ?ŠTð$ô3Í?ïÓØã˜Ó?€lJh?vŽ-ÑÞ¨?€lJh?ï÷ϋC?9?"Ž<®?QÜ`ƒÅg>?9?"Ž<®?ïÿo¬‹8Ù?ýh¶Žªl?
jÁîG»?ýh¶Žªl?ï#õ	¤;?³«ËQ¸ßy?›^Í0n	?³«ËQ¸ßy?ïÈpewö?}Žx\™D?{ÇÿË4@Ù?}Žx\™D?ït$¿þ?x]ói®—?ˆ¹"ì,—?x]ói®—AGN3FGL J0216.1-7016@rO}ŸÓo~ÀF—€"ØÀ:)ݨ½#À;äsùÍ¿å²Åz'ƒ@8"IÖã§@…A¯ó£¿æä""Ðÿ%¿ç­ëè	Øá¿ç:dUr«Í¿ÎaßÆ$@AGNbcu@…Š÷ÎÙ‡PowerLawPMN J0215-7014?ïÿ&¡Txþ?ÅÆñ¯…Ç?+Ûó¼M|?ÅÆñ¯…Ç?ïÍòÞ¤?ѧòÊ?yþ‹.œt?ѧòÊ?ïÃe§ÆûI?zaWì(œ?~M,r—?zaWì(œ?ïÿ7ž€g?	sg9P?GC¥À?	sg9P?ïþð—Æõa?Ǿ­¶èp? ö‡œgZ ?Ǿ­¶èp?ï\$ë¿"¸?¥•t?ôµë?"{b"£?¥•t?ôµë?弄hô@?/ï˙4ß?†Ÿ%Ñt?/ï˙4ß?ïðýÜ9QZ?W[8?¡}?^GC%»œ?W[8?¡}AGN3FGL J0216.6-1019@f"ž²gÇÀO闟ÄVÀ:.\|ÙÀ;â$¯â±;?åÁ&5ò@…¿1¯{@¡NÿÂmx¿Ý¦ë®±¦"¿ååënù\ù¿åå'Íò‰¿ïÿÇ|ÆAGNbcu@deF
¦LPowerLawPMN J0216-1017?ïþ´¹/¶ý?$¢9®Ä\Ø?$´k•SŽ*?$¢9®Ä\Ø?ïÀî‹t£ý?ÆÙ»5?ˆºdš}R?ÆÙ»5?ïiÁ}i&?†V˜&Í«6?'ÇÜóÂw7?†V˜&Í«6?ïW'ñ^Òs?rtS€"ñ~?•
¡ÎþG?rtS€"ñ~?ïüôèþ9_?@'ðß4?8Xº(÷ÅE?@'ðß4?îž^€ÐM?µ9"ÂiõÒ?¦ñGÝ8?µ9"ÂiõÒ?îè'óŽ?—of?¡wßsc<?—of?ëѨh-T¼?¤°8¡ÄüÃ?À¹^_J­?¤°8¡ÄüÃAGN3FGL J0217.0-6635@r%/€UûµÀH1" [TºÀ9 vö¢½À;±ù‰Ä9€¿Ùß-#û@…TøØþ?ÿ®Ó_Ž¿á
WÍ,ª¿âµ‹ñ¿×ôöí1Ç"¿â_O_¨uïAGNbll@ ßÙ‡+PowerLawRBS 0300?ïþï§BN¯?ì`êþ»?!Š%z™?ì`êþ»?ïÊtF4(?'ƒ
ñQµ?zÅÜÊo,?'ƒ
ñQµ?ï汛ª&@?u]úQ(]`?iNd!Ÿ°]?u]úQ(]`?ïýi±¹9â?"Â¯­L?4²sxY'?"Â¯­L?ïþdmys?&¨öY`¯?)¹+	F î?&¨öY`¯?ïE¹H¶}?±m°Í0؍?—PÑÁÆb?±m°Í0؍?ïánþA€?xþ9ž2¸À?n'<d—í?xþ9ž2¸À?ïëG57‰?XViÞ?d¸Êì2ÒÀ?XViÞAGN3FGL J0217.1-0833@eÎWà&EåÀOB:`NqÀ:^XƒNÔyÀ;åú÷''ý?çNáAsì@
F`·{@£, šTU¿ß}Z"õ?Þ¿ãl³vS]¿ç‹MF¿éùWÿ½²JAGNfsrq@',<žìÀPowerLawPKS 0214-085?ïç"9Ù¯?lA¨µw
ð?hlÆhãÐì?lA¨µw
ð?ï0Ýg_ò?™IƒË‰Ó>?™ü"J|ûÔ?™IƒË‰Ó>?ﺙՏÐ?úcšyñ?œh¬À&œ?úcšyñ?읖A(?"_Ï) ‹?»Mö¿Ì?"_Ï) ‹?îý³?ï‡?£0É3Ä? $Ì2Й?£0É3Ä?åÙþ‹á ?Ìퟑf€y?ÔLè<¿Ï?Ìퟑf€y?ëæ÷G
Ÿj?«þ2Æ1ðA?Àd"ãɂY?«þ2Æ1ðA?ÚZÓ¾·?´$—ÌÖV?âõҖ ¤v?´$—ÌÖVMIXED3FGL J0217.2+0837@c"4 -œñÀHQö¬m²À8Ï}š_'7À;X}ÞR0N?җæEï£f@&âÙ(¦@ÍnB¿âSï¥X®\¿â›^HhW¿Ûx½­mc¿æáT~\|XAGNbll@"º ě¥ãPowerLawZS 0214+083?ïÿÎçP©>ñÃ»9>øŒG¤üð>ñÃ»9?ïÊùú`?"J­hÒ~?zô]Þ ?"J­hÒ~?ïì»äŒ?gM‰¹e[‹?cD÷Ù{hú?gM‰¹e[‹?ïýè4ÿˆƒ?ĝ;?0¾X½+s?ĝ;?ïÿ¦•oW@?~&~ví?Z§d$µ?~&~ví?ïSšÖÒ×u?©UدÇÿ?•Œ¥)­S?©UدÇÿ?ïêR:¿/?p
\_š~?e­Æzà|?p
\_š~?ïúþ	Â?>>£^I›§?GëŸÉ,å´?>>£^I›§AGN3FGL J0217.3+6209@`™ÀµgU?îÆ)ñkÀ8yÛVÓKlÀ:­´{/P@îcßxv@
Ç`|?üÌÄ>]ß?Ø%‡P8I¿çQk"ôÝÉ¿î݆þâHµ¿æËW?4¦ÙAGNbcu@Šã›'·þLogParabolaTXS 0213+619?'ÇIJôtâ?œ¢"é+}1?ïiÁÚLßy?œ¢"é+}1?¥NIg'¯v?Á˜Ã…·Ì?î«i½ÞÈ?Á˜Ã…·Ì?×ßô½Ñâ?³Óbõåí'?ä¡—?³Óbõåí'?"ùæ^+›?xnȯ¹›?ï`0Ëé'Ã?xnȯ¹›?š°v<ã¯>?¦›ÿcø?ï*|MáèÆ?¦›ÿcø?ˆzº€?¥Ê~THöw?>àæ?¥Ê~THöw?×
»5[èš?½3@t9c?äy"eR³?½3@t9c?c.Ê=²Z^?Zm'*‹²?ïìÑ5ÖëN?Zm'*‹²PSR3FGL J0217.5+7349@`§Ÿì™ò@'ïÆ¡9¡À8šÞ>åÀ;_Ae%Ç?íxNµ¥@ì؏ù‡Á@BBàzS®¿çÉÍ#½R¿êv,g<$¿íNÀÉD">¿ïþ>F./
AGNfsrq@q;M@$³>PowerLawS5 0212+73?ïúÚD
Ì?@SCµÈgU?D—‡º¤òX?@SCµÈgU?ïëÒq?¨ŠªõSØ?œâŽUß?¨ŠªõSØ?ïÞñ^ôÏ?Êe&eék?D!бÊ?Êe&eék?í¥^´Ùˆ??aèóáô?²Õ+£;??aèóáô?ïñØ!6'ý?`~vƒb8?\O½"ü×q?`~vƒb8?ê¯ÑSð*?Ækþ±{Z?Å@º°?£Y?Ækþ±{Z?îXŒ)¼_? ©
'-®G?ªw=hà!? ©
'-®G?áé­ ·›?¶@cñ;ï?Ü,¤¾Éç?¶@cñ;ïAGN3FGL J0217.8+0143@dE– hUTÀK5[ßú¦ûÀ7̄eTîoÀ;"‹›˜?ð­¬
µe¨@A*»?†©@‹ jC@¿Þ›Rú¬a¦¿ã¢
ã%§¿â˜rÉ\f¿åè×}æñÍAGNfsrq@‰)gæšÔPowerLawPKS 0215+015?ïÿŠüÀ&î?	U]܊½?
@Á9Ÿq'?	U]܊½?ïÌ;	æe?Í×´"b?yâ{w}	 ?Í×´"b?ïړtïô£?qVïô™ÃT?r¶E"–¬?qVïô™ÃT?ïùž·¥?1¥oÌäTÑ?I… õÚN?1¥oÌäTÑ?ïÿ'²ø?
m69«ý%?SmÛ°b?
m69«ý%?ï,Ùs4'=?²Í‡Éí²;?šdђŽ ]?²Í‡Éí²;?ï¯dÌÞ?'?‡OŠÙl«?"&Ì̏£Á?‡OŠÙl«?ïô;Ë!ç?KkO›j	?Wˆi¢YQm?KkO›j	AGN3FGL J0218.1+4233@ap‰ßrïÀ1² Ñœ?À7Á¿ß~€9À;
~gäì@ˆĆØ@'Mp÷@ñ†‰qƒP¿ÞíC7À¿+¿ä_rÆ	ÿ¿æS=nj@¿ëöDyùã~PSRPSR@†ûuY³Ð}PLExpCutoffPSR J0218+4232?‰-Ê^J?•€t0]Ó¶?ï›HÖ]š:?•€t0]Ó¶?­Ó"\?¨‹Éf)Ä?î"Ï㭎ï?¨‹Éf)Ä?Бc¼Çz?±œjÖÎÞ?ç·N1!œC?±œjÖÎÞ?Ôâ»'j?u˜]~;<h?wº7?u˜]~;<h?{ògKø«À?'ýTkr'ê?ïÈ1V0±?'ýTkr'ê?™Ô"Q2ø{?´æÑÁ?ï1[Ývh<?´æÑÁ?³4锌G)?¦™ÄÍ$
¡?í™bͳ/J?¦™ÄÍ$
¡?^t¤á"‡?TdŸˆ9Ó?ïðÅ­sÁ?TdŸˆ9ÓPSR3FGL J0218.9+3642@a»»ÿŠ;À6ì¡`7x<À8Û§¦¢–˜À;Ccf×¥n?î3·#\m@‡¦ÞP­Â@› ¿ã…Ÿ cš&¿è…Ámüg¿æªÊo‹Q¿ïÿ؍ÚAGNbcu@‡Ÿ—Oß;PowerLawMG3 J021846+3641?ïùsZç?XÅnç\M?J3®Ë@2?XÅnç\M?ï¼]#¸î?"¬5Ao$ë?€è·I7îb?"¬5Ao$ë?ïxSLÇóŽ?|ã^¥ÏøC?õ–h¹\@?|ã^¥ÏøC?ïСÍ~?Uï zÌy?w¯~²á\Ý?Uï zÌy?ïøæÉM;r?Pá:§A?Ldۊ?Pá:§A?ïïœkÂ,?¬\é÷Sp?ŸBw¯$u?¬\é÷Sp?ïD¼sŸp.?'Xê=P6‡?—hq'9d*?'Xê=P6‡?ïX`'£?'Õ¶%¤}ñ?"óí°Ä™Ó?'Õ¶%¤}ñAGN3FGL J0219.0+2440@bbÇÿÞrÀAGñQçÀ:Oá4bÞÀ;ÀËÈÀΒ¿Úo3˜@^¸»F=?ý¶ô ü9w?ï¿J£!¿åo7ýr\¿Õ	äEöj'¿ÞšR=ÜÑÊAGNbcu@±@L‹C•PowerLaw87GB 021610.9+243205?ïÿ©Ĥ?
ßL¼?¹ê¢Ãµ\?
ßL¼?ïÏEÅÜîƒ?'¢»q"î?x]	^ˆ?'¢»q"î?ïè˜5?bx9@ù?ggþåûQW?bx9@ù?ïþB^'[?ÍbŠ:v8?+Ú:·R?ÍbŠ:v8?ïÿف2'ð>ñ0õ²£>ó?vW~'n>ñ0õ²£?ïD-^‡õ­?±"ä m?—zT)Ùà_?±"ä m?ïéí
=æ?kŸÛ:kfK?fö';9±?kŸÛ:kfK?ïöœ»ÑÂ?GvSÛñª?SôÆ(­e?GvSÛñªAGN3FGL J0220.1+6202c@`¤4_½Œ?î(ê@6b#À8ò=)HÏÀ:FÁÅ1ÍØ?ôܽîbž±@>jÉÍhÿ@\[ÿÛ¿ß¹¿³4¿æà± ÷[í¿æé  0ø¿ïû†ô{gOTHERspp@¯B¯·éPowerLaw0?· ӖŸÒ?¾'ÎÕTt?íåGO?¾'ÎÕTt?Öi(v>K?ËròÄ`Ë?äËkôDàÛ?ËròÄ`Ë?Ü9~êt[$?µÈ 0¹:²?áã@ŠÅÒn?µÈ 0¹:²?áœDu60?®@æ±¼D?ÜÇw"ß?®@æ±¼D?Ä$ß<Ï?œ`éÚÀ!?ï!Þ¢Z?œ`éÚÀ!?±z0ʄ:?¹ág¬•'x?íнúêÈ?¹ág¬•'x?˦óû9ó?µ»¨•cÜ?éC1ƒ?µ»¨•cÜ?ÁEaá÷K?§ÎÛ>v?뮧‡»B-?§ÎÛ>vMIXED3FGL J0221.1+3556@aÓjßqêÿÀ7{/à˜[¬À7œë"aq4À;
.óŠ§¿ìc²‡QB"@Š|p>@A(ƒÓà¿ã'›ê'ì'¿å¿aC*»Ú¿áùx¸‰°¿ã£ˆŒ<JAGNFSRQ@"í(ŒçPowerLawB0218+357?ïÿÆÞ—/>ù&͛2>ü' s<¼>ù&͛2?ïÚ¾Wi{?|uºÅJæÆ?r Ôgžf?|uºÅJæÆ?ïâw["²Õ?t ÏÞB²?mˆ¥¦Âæ?t ÏÞB²?ïÿü©M/¢>´ÙLûklô>º¶ºøsÑÆ>´ÙLûklô?ïÿ8×Ú>?!EV¾?±¿¶6‹|?!EV¾?ïdX£Éâü?£lÔÏܓî?"tëäh?£lÔÏܓî?﹓"¬¢‹?…ÌqÜ[ù
?›Òo£M?…ÌqÜ[ù
?ïÿñí.é>ޒ5‹çéc>Ü%\`áT>ޒ5‹çécAGN3FGL J0222.1-1616@gÉ hUTÀP—L?ß À9|ÙGdCÀ;Ê+÷Տ?´Æ;'õÙ°@˜Hí¯›d@ÎñŸêìs¿ãìå5ú7ê¿èˆˆODa¿éënÆåµ°¿ß~ý<'h´AGNfsrq@°Ù_í¦aPowerLawPKS 0219-164?ïÿÑ~Y>ú¯ ò'|>÷r¡\·:ò>ú¯ ò'|?ïß<6Î.ˆ?| ³'¨?paäxœh;?| ³'¨?ïÇ2‡ÍÐi?¸å¿Uùƒ?|f¼w£n?¸å¿Uùƒ?ïöpM#g?:'L£Žn,?Se1óA%?:'L£Žn,?ïÿž9w¬?	$ðÀE×b?q'P{#d?	$ðÀE×b?ï%8ÇÜ?±':¼Ëj%?›_øúWh?±':¼Ëj%?ïÈ¢""EB?{Z;kœø?{®¶T™ï?{Z;kœø?ï˜!͍ń?{2"&9ý?‰÷ŒŸþ;?{2"&9ýAGN3FGL J0222.6+4301@a"Р+"À0ÄZ&–mÀ6]<¼HñÀ:
©yámn?ð‰•*6¢@$}õÏ$–?ýTÛ+µ:Š¿×>5фRÇ¿à¢L¢V£¿Üa|…Z¿ßCb¥ç…¶AGNBLL@Œ"û²þÅmLogParabola3C 66A?ïÃÜòšøÐ?…‡Wõ×?~†²ƒ—Ç?…‡Wõ×?ïÉýaÙ?j קK}?{w^Ûg?j קK}?í³´˜"¡?©YaÇÐv–?²b[=¡Ü?©YaÇÐv–?ïÿ}"vl?D©3F?M•è3¯1?D©3F?ïá¿×µ¢Ó?nr篫ò?n@(aº"r?nr篫ò?ïˆ÷œ"?¯´—}ï?ŸŽáíp?¯´—}ï?îÕL³Àiñ?žšÃ‰Xä?¢«4ÂA'ù?žšÃ‰Xä?ïÿ'a8v‹?Ùï–~(?g¦9Ùvþ?Ùï–~(AGN3FGL J0222.9-1117@f @FA-ÀO¦ÄŸ×¡<À:h|°TÇÀ;Í8Ëùh6?"z)@…Ë[ˆ'?ý'ýŸþbœ?ïàMH欿ڝû'¿ã5Ÿ°E>¿Àa
ÂAGNbll@¯cñA PowerLaw1RXS J022314.6-111741?ïÿEnÛ*?ƒd|ƀ ?\Ÿ¦>?ƒd|ƀ ?ïÓP ÌË?=3ð¥ø€?vWï±MrS?=3ð¥ø€?ï×P#âeï?j­Z5g€A?tWî*Ièr?j­Z5g€A?ïú—
"Re?3Õ
$s"?E£Ëp'%?3Õ
$s"?ïþÌ#ã»?!ßùf›å¶?#=¾¹w@?!ßùf›å¶?ïU仫è&?«îˆ‡™)?•Chªe@?«îˆ‡™)?ï­Ðû'~?'oÀ‰æù?"‹úA '?'oÀ‰æù?ïÖ#¾í;?m.›8¤?tî1Êò}?m.›8¤AGN3FGL J0223.3+6820@`hğס<@ãŸú[ÑÀ9¸À*'À;nºeÁû¸¿ûт"|ÿ@¼×ŒCp?þ£¿à€2ë¿èðÁFóµ¿Ø}j-4/v¿Ü¬è6ÆÌ¿¿ßšØŒ&GAGNbcu@µ‡yÛ"ÐåPowerLawNVSS J022304+682154?ïþÉ1æ"?-üFEâH?#lñO'Ø+?-üFEâH?ï×T˜¼,Ÿ?|*º,ýà#?tU³žzs?|*º,ýà#?ïå÷\²!j?l¶Ò-—j?j£^\¶H?l¶Ò-—j?ïÿ÷¼1™>È4Áñéhk>Ї{õ÷¯%>È4Áñéhk?ïüÚ)4_a?2"½FzîH?9.¸:5Æ?2"½FzîH?ï$´y¹!?¦'Úêdß?›i9_á×?¦'Úêdß?ïÚëõm;(?vžÔ~—?rŠTa+î?vžÔ~—?ïÿoâ;?V‡gãØa?¿ý4<0?V‡gãØaAGN3FGL J0223.5+6313@`¢Í œÃ@ye`,¨À9 @ŽÉ\À:ãPl)?ø‹×D;@uÊ\…!?þöx¥-K"¿ÚAøW
æ¿æ0NÃÌ6ê¿êö‡uœ©¿ã"øSIQAGNbcu@'ôÖ¡aåLogParabolaTXS 0219+628?é=MSx€£?Ês̑¥?Ë
ʲýu?Ês̑¥?Þ™äåiÉ?ж½œ-G·?àý3
K?ж½œ-G·?ë	ü²\wê?®eLhˆN?ÃØ
6Ž X?®eLhˆN?äkÍJ?°ÈaÙéß»?×(ekáòÆ?°ÈaÙéß»?ר÷q)þ?Ð$D2?ä+òGk?Ð$D2?³¸næ7þ?»Ÿ
·M´"?íˆò#bI?»Ÿ
·M´"?åëâL÷ç?¸hý©}V1?ÕÆ(;f3?¸hý©}V1?Åd7ÇÁ?¶¢\w—i¨?ê &ò:Î?¶¢\w—i¨MIXED3FGL J0224.0+6235@`«¢_¦XÅ?ùáVèˆ?À9	"EœÂCÀ:lï­¢e?äc#c1}¦@tk0$µí@Íê€d?Øòtý¿çeg˜•›¿ëºÜ	€²¿âÑäÏ"£OTHERspp@žv<ÓZ…ˆPowerLaw?îšQôÙ/?³ì©¨Æ¸U?¦Z౒&?³ì©¨Æ¸U?ï[zË*éÁ?¥5—Ví?"¦—3+ß?¥5—Ví?è×YŠ­:?³¥º3¶ôp?Ì¢™ÕKù?³¥º3¶ôp?ï	e7£k'?"Â)j8F?žÓYû‡ö?"Â)j8F?çUS&?ÌÆtä-'‰?ÑUáY²ßø?ÌÆtä-'‰?ëhÚ!ҖC?ÃÍGÈà?Â\—xµ¦ô?ÃÍGÈà?â#Å—µ$?¿â›&rÁ¥?Û¸uðЕ¸?¿â›&rÁ¥?éI
`V,?·Úà¾t®ù?ÊÛãÖ~§P?·Úà¾t®ùAGN3FGL J0224.1-7941@ržq_ˆü"ÀBAÉ¿Ò‡À:ÏO^À;ÎïS	'¿õuŽ²Š×4@-#""±Ö@ÔÏbpã¿égØt~_µ¿ßÊ1%€±Û¿Ú÷sË:Ñ¿ç‰Äl'6AGNbcu@™5y	k¹ŒPowerLawPMN J0223-7940?ïýÛ¾éE?,tfI^ð7?1"âçüÈ?,tfI^ð7?ïÙFãò¶Ê?ˆ·f&Ú"?s\ïGC1?ˆ·f&Ú"?ïãw ÂÐ?iRÃ[[Þµ?lˆ_LN1Æ?iRÃ[[Þµ?ïÿÆfM´5>ñ	A¹PŒM>üÌõÎ:>ñ	A¹PŒM?ïüþeÌ³?8ä0Ã(}?8ÒÑDo¿?8ä0Ã(}?ï6¬})©û?®`ŧ9va?™*pZÊÀ?®`ŧ9va?ïÐRéºvç?€aST­Uµ?w֋x8u?€aST­Uµ?ïü–nõ^Å?5²&ú÷e?;Lˆi~ì?5²&ú÷eAGN3FGL J0225.2-2602@jéÂ?«ºÀQA×,uªÀ9C[m TÀ;ÚºÌH¦?㧦¤¼YÚ@‹úÇ1€@NÌÀb†2¿æoû
¿è™›fÅ©9¿è<Éøj¿ïÿµððÌAGNbcu@yu­­ê‰PowerLawPMN J0225-2603?ïÿmöu	9?¥²´~?A,þª/Ë?¥²´~?ïÌð(qŽ8?U;Ö Üº?y‡ëÙÜ	?U;Ö Üº?ï«îQ=¤?pú:®#¬¿?…k´(ó?pú:®#¬¿?ïöøyӁ?8£ån'Yw?R
»\¾n?8£ån'Yw?ïÿÅÚ.#?%°°gý>ýþX-¾â?%°°gý?ï_˜P³?ªLÌ®1?"Œòz?ªLÌ®1?ï¸&ύ±?€`ÿ€õz?öL3õyä?€`ÿ€õz?ïݦèrÖÈ?býî?Ô¥`?q,‹×»¹?býî?Ô¥`AGN3FGL J0226.3+0941@cŤ p¸ÐÀGKÏ`%ÆÀ9'y…ýÛcÀ; dYEìs?êÐæ‹Kx@Aw÷ˆb@}±ÿlc¿"£úhóŒ¿èFwÓÌu¿ÓE
MXDÝ¿ëjò›Ø'
AGNfsrq@•›Ò×süPowerLawPMN J0226+0937?ïýÉF».?0·í&¤4?1·9Þ
?0·í&¤4?ï̦¿ÐmŸ?ŠuÀ´V-?y¬ kؽ?ŠuÀ´V-?î"ÖcùÎ?›e‹ŽØº0?§²™ÊàÇ'?›e‹ŽØº0?RWs?f^÷8††?‡•kwøS?f^÷8††?ïýõ—Ø_Ž?3'a0ør?0S@…e;Â?3'a0ør?îýá"|p¶?²¦ó¤hZ? !æ·]
?²¦ó¤hZ?íáPáޛ›?¤[¼¸^Â?°õxïSU*?¤[¼¸^Â?îðð"g^?û|áȟ{? ðýØ®8?û|áȟ{AGN3FGL J0226.5-4442@p_
߆ã´ÀP̀SÀ9ÙLvѵÀ;¶³ÑSDK?Ý~-Áü‡@É.²E?ÿF]7ãq¿âYËRE¿t¿è¯ÐôéeN¿´y´22hn¿ÛþÍýñªIAGNbcu@£viᰉ PowerLawRBS 0318?ïÿl´???P} ™½?Š"ÆՆ??P} ™½?ïÙ½…©o?"ö<õv1?s!=
â"?"ö<õv1?ïîiÄÎô?h@a
±0?a–ä8q\?h@a
±0?ïégÅ f?OE³vùX?f˜:ê!Êh?OE³vùX?ïÿ	4~"7? x³:ƕ?Ùu@垎? x³:ƕ?ïGû¾'?§ù`Ëê4?—€ƒõ?§ù`Ëê4?ïß²rƒ€(?z®ܹ¸?p&Ʀâ"J?z®ܹ¸?ï¬fpªë"?v¬€Ûîaø?"æcÊöK?v¬€ÛîaøAGN3FGL J0227.2+0201@d¢æàé´ÀJh˜Ÿž–YÀ9¦Ž.+ŒvÀ;¨è»?܏?ÐSkŒ–@	éôZ@VOàh
*¿äÂÖxênì¿ã¥ªbÙX¿Ì~ê­¥¿èîðL7AGNbll@6oPowerLawRX J0227.2+0201?ïûžCÍ_D?Dmaiý[Z?A†ðá™ê?Dmaiý[Z?ïÆ%ÁˆÃ?…i»B|?|íp(چH?…i»B|?ïڀX2q?t‰<N!8?r¿ø×Vcp?t‰<N!8?ï˜Îèƨ?qžÉ`Þöq?‰Ì|ÖüaÌ?qžÉ`Þöq?ïîíwMz˜?d½¢"Ç?aˆ¢G¹?d½¢"Ç?îâ"C"?°çƒ÷å·ý?¡ß
Ü«tà?°çƒ÷å·ý?ïnñ£¬ÿ
?'ͯ½ö¯Å?'!ˌìT?'ͯ½ö¯Å?í{çd}®?£â•ô¹ôÛ?´ ÄÛ6¨ü?£â•ô¹ôÛAGN3FGL J0228.0+2248@bɸ!ïÀAq[ßú¦ûÀ9´Á"tŸÀ;–[ßú¦û?ã›@§~ÎV@z¯Èe@öÿ /Å¿àÄø5û:¿Þ*ÀžýAñ¿àøº04s¿ìÌã6àVAGNbcu@˜Ú­BÃÉïPowerLawNVSS J022744+224834?ïóá[¦ò?W€€™œŒ|?X=IZ¾œÆ?W€€™œŒ|?ïÆe>?Ù-@EŽ?|Ía
á;?Ù-@EŽ?í¢Ùšqä?¢×DŠs‹é?²é7ää>Û?¢×DŠs‹é?ïÏ¥.D®R?Ug{¶s?x-hÄ;»?Ug{¶s?ïð1Ÿõ?b=‹{ɤú?_՝á¾Õ ?b=‹{ɤú?ïƒ/'"u?±§jŒ)³G?œïšUÃT?±§jŒ)³G?íówû}þø?¢,?Ÿ¹T†?°d@%ÇÖ<?¢,?Ÿ¹T†?ï&t"¥¹¸?…¾ö¢¢?›1m‰úô?…¾ö¢¢AGN3FGL J0228.3-5545@qc²?î,™ÀL<—à[õÊÀ9!Å;ÞÓ`À;Ë®4[Q_¿õcl´3Mà@÷°(§>@h)@@6ý¿â}KÌ ñÁ¿æ'
ÏfÛ¿äŒR•	x5¿éö¥8^@AGNfsrq@ƒo
_™Ã‹PowerLawPKS 0226-559?ïÿ*¯ø>?`«OU?ªËÂÙR?`«OU?ïÏ~ÿu§³?¦†îÅe½?x@€4®ˆ?¦†îÅe½?ïãój_?ilM?lÿä"`¾?ilM?ïÿÿL¯c¹>×¾UXîd>–g>æ=4²>×¾UXîd?ïÿm(Õê¶?¼aY*ÛÁ?Z샐z?¼aY*ÛÁ?ïE—Úµ²?±·-ùn|?—MD©I²?±·-ùn|?ïÀ¯àªÐ?ƒóæy§Ò?¨~ý´?ƒóæy§Ò?ïÿü=côØ>Á^ï/"ï>¾Ҍ»3>Á^ï/"ïAGN3FGL J0228.5+6703@`†‰_$RÆ@Ë# C+úÀ9‡½Q.ƽÀ;6O¥YÁ?½Š|lã@
òê|‹ó@ó° ™¨ˆ¿Ü@YM	"I¿ìP|V¿à*rހ¿¿ïÿ€m•AGNbcu@ƒŠû"ŠPowerLawGB6 J0229+6706?ïåzìbòÇ?kÌÉön¾?j…yQI"?kÌÉön¾?ï ÐRqr?v\J%4?‡Ëë‰"€?v\J%4?íÕQ˜E~?œìgíò6?±Us<AÓ?œìgíò6?ï_âÑpöb?y–CÀ vß?"¥Ð)e¹?y–CÀ vß?ÂZó?'@&ÃØ?‡Y~iCT?'@&ÃØ?ìñÃW¿?Ø?¼ÊL÷¡Ùü?¸qåBC?¼ÊL÷¡Ùü?ìUx-ëW?§¹ß÷VK,?½T>—P¥E?§¹ß÷VK,?êU¦âFJ?°÷}³ž£P?Æ©dvæÕü?°÷}³ž£PAGN3FGL J0228.7-3106@l«µŸôýmÀQ| À:Èá!§¼À<®ÎµY¿æ2¤[Ù3@d
‡ÃXZ@s`ù•¿ãóåVO ¿å'™³£c¥¿ÐZJÂN¢-¿Ý83<ZAGNbcu@Ÿg8†YJõPowerLawPMN J0228-3102?íPRº"m?с
/ó|~?µek㪔?с
/ó|~?ïØ£3üS?†–ZÂ:Äï?s®wXóRp?†–ZÂ:Äï?ïºÓÍ$á?†:S
?K7ü蓾?†:S
?ïþŸ>ƒ¯?€ì8€œ?&b;?€ì8€œ?ïô õVs?v E£'?W¿ñË‹9?v E£'?ï\Å+ rÅ?©òÖnVã?"gZ›ñ§f?©òÖnVã?ï‹5N| ÷?•,\b¶?2¬rÎC?•,\b¶?ïó	è?Qjo3ŽR·?YÁñü­ø8?Qjo3ŽR·AGN3FGL J0229.3-3643@n~9ÀëíúÀP̖üõŠÀ9&D7guÀ;ËW`9%»?á¹ØRUÒ@½º@N@Oß_¡{:¿äpô(G³¿æ"þnIM–¿èÓŨôe¿ë¸V5õ8AGNfsrq@~p#9ÀëîPowerLawPKS 0227-369?ïþó¶Ã?&‹"kéÐ?/ÐÁJU?&‹"kéÐ?ïÐóÔ^ͧ?·Í¸åL;?w†ݧ°r?·Í¸åL;?ï¯tŠŸw?y&ÝôIñ?""ÝZý'>?y&ÝôIñ?ïþàŒ-†‡?"Ö¸ÖÕÿ?!÷;;öÅ?"Ö¸ÖÕÿ?ïþ´	¡-Q?%#I#·AÒ?$¿aÖnÉÛ?%#I#·AÒ?ït"òºê? &ø¯'"Õ?'|/j?¨¦? &ø¯'"Õ?ﭑ6[K?'é:³†‡õ?"›¸èYh?'é:³†‡õ?ïüã,¬þž?0ӌÎV<w?8æ™ÿ6
`?0ӌÎV<wAGN3FGL J0230.6-5757@q…E€<ÑBÀKL®¿›‹âÀ:Ç1Ç"háÀ;í´£á8?à _ŒúÇ@¬²£UÚþ?úõ@|òÅ?ßîCÐuº¿äÝþùDп⏃0 ¯"¿æ5²%AGNbll@ÀíRÐå`BPowerLawPKS 0229-581?ïþ·¿äé?!ÇÝë[¬?$"ßçw?!ÇÝë[¬?ïÍrÛX›?ŽRÝÒÁs÷?yƟb6¦?ŽRÝÒÁs÷?ïÕïD›æ?qE(	Pº?urˆZò\Ü?qE(	Pº?ïéÙbe?TV÷"/n?fâ&͵…&?TV÷"/n?ïýãyÁ?/Ô }ç?0çƖ$À?/Ô }ç?îÛQ!'9w?´®:',zÎ?¢JíïD6Š?´®:',zÎ?èØF(?ˆ@^¬î?_¼0(?ˆ@^¬î?ï)ÐåÏì×?"îÆ÷¿¢i?šÅãLá#?"îÆ÷¿¢iAGN3FGL J0230.8+4032@aÓdÜY2À2€nÿ'÷À8ìÓXØjÀ;ž–"ì"?д>Ç¢'@z›Alo@e# ™5¿å©À‹Ôg©¿èqSlŽž"¿èé"¡¿ÝûžaTƒ»AGNfsrq@0U2a|PowerLawB3 0227+403?ïÿè"?ç2>s±à>þ+ñ[·ä?ç2>s±à?ïʯ×Ç/?Ž6›a^®{?z¨w|$s?Ž6›a^®{?ïßIFùlF?f‡N"`ð[?p[\•×Á?f‡N"`ð[?ïþÑL
t³?œSŠä_µ?"ëBwTr?œSŠä_µ?ïÿ5Ëúûð?k^Wóy&?FÝ›UÝ?k^Wóy&?ïô»˜
è?¯|訢?Áh'&ù?¯|訢?ïÀä&‡Ì?ö
I$ó;?ž-øjÆ,?ö
I$ó;?ïú9Îǒ•??™qX®?GÄ7Õɛ??™qX®AGN3FGL J0232.8+2016@cýŸÓo~ÀBNº@NÀ:"7ÜæÀ;¦7¾³.–?áæ'²ƒ@)@Í$¶n@4ßxöâ¿Áô©Ú\ ¿èßiKaí¿æ¤ç¢Þ^¿¥g7"
`AGNbll@«†Â&€PowerLaw1ES 0229+200?ïþ¤ŽrҎ?)î"I·¯?%·çêÑ?)î"I·¯?ïӗ"ôúq?Š6"ê?v4=xtC"?Š6"ê?︔èɜ[?z)RM™²?ÚÅÌ9a?z)RM™²?ïìUøÏE?P§õøI8<?cª~;jÊY?P§õøI8<?ïû]èNĚ?L'WSüð?Bˆ^±#	Ñ?L'WSüð?ï3Ò¤kô_?¨×2j+/?™…«oØ0?¨×2j+/?ï"½G&c?—
í§*)?h_²9›?—
í§*)?ïCm…ž?=ŠB_?—'O`Uú4?=ŠB_AGN3FGL J0232.9+2606@b·žÀµgUÀ?n¢ ©XSÀ:Š°¬Ö)À;ÔîµTá?ݑwÿ‡o@.Ò¶p¿Ü@°ßŸã4ÿãë`FøÉ¿×Zp,>¿Ýc²£<ì¿ä§¿ zšŒAGNbcu@¥lÅýŠÚºPowerLawB2 0230+25?ïþßöd·?Iä÷yŽ?"–ˆ¥F<?Iä÷yŽ?ﲚuGæÛ?ԕÀ‡t?ƒYbµícK?ԕÀ‡t?ïàY
&H?c#¬çÛð!?o¦ò¦ÝÆ6?c#¬çÛð!?ï@bUµ"?u
	!©Ž?—ÿÓ±Ù±?u
	!©Ž?ïûÚ»f·´?>3&à"?@•Hº'¸?>3&à"?íŠÈ£ûÐÏ?ºLXUµ?³©ºákT?ºLXUµ?ï³
²®Ð?'à¸U15Þ?ƒ<¸X{¶?'à¸U15Þ?êS¾¹Â6¤?«½ujg?Ʊ÷%o?«½ujgAGN3FGL J0236.7-6136@q³SX"ÀI¦Ò?ÓT¦À8…´~êÂÀ;"Æü©3k?ç}¹ÝÂúw@äÇÉ@w:ßyø"¿àp°F%ˎ¿æ£ªGDk¿áހM¢A¿èˆ4X'AGNfsrq@…/	"SPowerLawPKS 0235-618?ïÿT¤GŸ?*›PAóÍà?k|ìHž?*›PAóÍà?ïâŠÎ•?{7ò!}x±?mu1÷q*®?{7ò!}x±?ïáN^²½Ø?n(H'pؔ?n±¡:§½?n(H'pؔ?ïÿí9L°>Õœ~¡}>âô°r›øõ>Õœ~¡}?ïÿ"Ç2Ú?Š0y³Ê2?Ü­&«?Š0y³Ê2?ïTX	´è2?«¸¤²ã}Ï?•tþÇ«+¼?«¸¤²ã}Ï?ï–â"ۈc?‡Å7>?ŠGwLƒS?‡Å7>?ïÿî-"Už>àæë³ö#>áÓ!çƋ±>àæë³ö#AGN3FGL J0237.5-3603@n%ËßÒcÀPr¨æj-À9êøš°ðÎÀ;ªÞüz9'ÀëhnSp@®xù¼?ý»Ð@Ô¿Ôûè]ê¿ÚkNûï,ҿґ*2w¿âÞM[ä"yAGNbll@ªÂ÷KƧðPowerLawRBS 0334?ïþñ—ÝVÞ?0ª½Qª? æº[q?0ª½Qª?ïÝ3ğùý?ƒÍµM$s?qf¼a™E?ƒÍµM$s?ïáôؕ¿?d+¾¦?®?n'/'¸'?d+¾¦?®?ïÿÿaÝ>£"¾¶Ê2>"Øi½û>£"¾¶Ê2?ïþ?±ê'?&xq…x'?,ït'â?&xq…x'?ïU_Z®wL?«´]Ö?•T¯X€q?«´]Ö?ïÖVþhª?vRÕ°Ž7B?tԁYŽþ?vRÕ°Ž7B?ïÿóƒxx•>àlù)×>Ò>Øù¹>àlù)×>ÒAGN3FGL J0237.9+2848@b¯8¾øγÀ<…'ßBñÀ6ë7OËÀ:ûìƒKy@6?çÍ@ h(,ºž@*%³Bâÿ¿áêÀӚF¿æžºæÎß)¿æŒ*Š¿ê½ucÚEAGNFSRQ@tf'=[«"LogParabola4C +28.07?ïôhM­n?kãóI/î?W/dkjTX?kãóI/î?ïÃ|Àߝy?R6³º?~AŸ|C‡¾?R6³º?í†
óމŽ?£íD6qÉI?³ÏbÁ?£íD6qÉI?ïþBG%[?o4UPÌ?+ێ;‹[ò?o4UPÌ?ïç+Pn`?hËJ{u?hԯ̹:?hËJ{u?ï"¡šÚ?³˜Ù"Œ?žk壪·?³˜Ù"Œ?îcò{»•Ë? ©Y-,U?©ÀØG¶?E? ©Y-,U?ïÿ8JÛVº?|ÃWOâ?ö¤ŠÕ?|ÃWOâAGN3FGL J0238.3-3904@nþã€ßÀP0‹À'¢ÜÀ:uå"m/®À;÷©4AP,?×Í/@Ð溉©7?ÿ] D-¬?ï÷½À"-æ¿âÕ -qþ¿Ë\6;ÙÓ¿ç8€šR¸AGNbll@¤"þžšPowerLaw1RXS J023800.5-390505?ïÿçÒGò?ºôNÆ2'?ƒüvTÍ?ºôNÆ2'?ïËåئ9?‹N£‹ f?zq3IK€?‹N£‹ f?ïÚíE?oß¼óˆ?r‰z7­H?oß¼óˆ?ïÃA!¢*ü?b¸ekMƒ§?~_o>ɲ?b¸ekMƒ§?ïýC ªß+?7³Œ®0*?5æùJH#?7³Œ®0*?îýêžïÄÉ?±B†˜xí? !Vߚh?±B†˜xí?ï¾»ýq°G?€æËð¾¢r?€Qšüèk?€æËð¾¢r?ïò

?‹`ÜÖވ1?A¾ÃS?‹`ÜÖވ1AGN3FGL J0238.4-3117@l¯¬ºËCÀP•‹B¹À9XõL»šÀ;hœøɪÙ?Íè»q@ñ@áü]‰ ?ý^%y¿ÒúÁ?ƒ2¿ã
ù;H^¿Ðá¢Y(1Å¿ÖwÑýÅ­AGNbll@¤ezxl"PowerLaw1RXS J023832.6-311658?ïü]Sm:k?HÚT…¬?=f]_K—?HÚT…¬?ï˸g\|û?"-F<$s?z#Ìsm®W?"-F<$s?ï×Ï%RÜ?kÕóxó?tmt£@?kÕóxó?ïí
÷Tá?Hî‰HÖc=?büõëoW?Hî‰HÖc=?ïø©/ÊÚ?MSLx¤?M[A'Ðh?MSLx¤?ï ãÞóQ?²œâÍU?›þ…ÙcØ?²œâÍU?︧7«¬°?ƒb}kí?Ö2
n	õ?ƒb}kí?QŸQa?tÄôý¯ó?‰•+Šm7Ù?tÄôý¯óAGN3FGL J0238.6+1636@c˜à¿]xÀCÏߦÄ%À74^¬]ÁÀ:¥žÜÏyO?÷³ÿEÅÝ@!M^|Y@…Öí¿Ý諍ën+¿ãÇoܘ&¿â6"׿æªÒîò3AGNBLL@}"¾ß¤?æLogParabolaAO 0235+164?ïþg³?,c8ºÎï?)ƒÖ†6?,c8ºÎï?ïɝýETb?'/æÄçóf?{1i{
?'/æÄçóf?ï Q¨$ˆ?ˆV°%
þ?‡ë–œnw?ˆV°%
þ?ïÿûn(…8>¹õ–gȳ>ÂFúUðÍ>¹õ–gȳ?ïûfTëI?D»Ø~º<5?Bf¬2ç=?D»Ø~º<5?ïlk'v?§â¼bÇJ'?'r®ŸB?§â¼bÇJ'?'¬ˆ?‹NiÁûè?‡"¾Ø%B?‹NiÁûè?ïÿþ±‡ˆ0>­'Íô>¤çŠÕ#j>­'ÍôAGN3FGL J0240.5+6113@`õ¹pޏ?ñada(ŽêÀ5xþ'jöïÀ:%ÂÐʈO@K4[Ò9@]Ë5ó×Ô@N
Óî$¿Þ'Q¦»Á¿åt÷ù¡A.¿æÉÀµg¿ëS?bk…	OTHERHMB@¡Z³LogParabolaLS I+61 303?ï!"Ò	o?°ã'µ´?›Û¥·òæ‹?°ã'µ´?¹ø"µ
?Ç+Ô~5Ô½?ìÞÿ€íêî?Ç+Ô~5Ô½?áQ¨¶ú°?ºw{Œ"KÍ?Ý\®"ô
¡?ºw{Œ"KÍ?Ŭ͠S¿?²ÁÍ8ò(Á?ê»Ô̗ë?²ÁÍ8ò(Á?ç–«´¾?Ê|7©9Ÿ´?ÐÓý𨖄?Ê|7©9Ÿ´?¸ö:zx?ʈ\ᾇ¡?ìá8°†×0?ʈ\ᾇ¡?㩯æ%þ?Â]q­
â
?ج 3´õ?Â]q­
â
?¾|\?ÀE+Všì?ì>°t|?ÀE+VšìMIXED3FGL J0241.3+6542@`½œÁæ°@Ñu @&âÀ9>$'ýÀ;9ݾŒ˜)¿ð Õugá@{«Ý>@£Gßg¯¿â:ê«@FR¿ãu.å4'q¿á}.\'[¿Ôb³ðC/¼AGNbcu@¥ö¦?PowerLawTXS 0237+655?ïælÝ_'?"›±CPÚ?iû"$°•?"›±CPÚ?ïÄRK1#?'º'›OO"?}ÖÀ@úR‹?'º'›OO"?ï|ŸÓß?‰¼9ñW5?}¬$Ìî$?‰¼9ñW5?ïþx¿À…þ? 9W`ÇG?(tÆßæñ? 9W`ÇG?ïëü@5'Ì?`1öh?d¿Ãû³?`1öh?îíÕÜs'{?®þEqҕ?¡"¢8ÆèT?®þEqҕ?ï	oˆŠ?•G‹EH'š?žþÜsƼ·?•G‹EH'š?ïۍWÊtá?o¥ž,tÖØ?r9T-Ss8?o¥ž,tÖØAGN3FGL J0242.3+1059@d:¬ÿ§ëlÀE¬×5ÜÀ9£YË8À;–¥€éŸ?ñäŸANSö@Xéçå¬î@N_ƒô¿ãÔ—m[¿å³{œGb¯¿è¶8¤ißË¿ïÿò"5£ÀAGNfsrq@'
æšÔ,PowerLawOD 166?ïÁ¾HÐ~]?Ž°éŽÆÏ)? Û|óݑ?Ž°éŽÆÏ)?î«»ïs¯"?¢éh†H¦Y?¥DAéÂ?¢éh†H¦Y?î(¬
àY?¢ã÷??›?­5A	Èq?¢ã÷??›?ëðGšÒ?•Ãûå¢à?Â>ቔ¶?•Ãûå¢à?ïr}¨f*?¦fN$¼}?'°QÒr¹?¦fN$¼}?çoÆÏ\Ê?È#C¾"œ?Ñ!þraFl?È#C¾"œ?ì5[ÎÕ2?°G1¬S?¿îU!‰Vo?°G1¬S?ÜTæ˝ð?±›jì°?áÕüš1?±›jì°MIXED3FGL J0242.7-0001@e"-@ªêûÀI÷˟¦#À9°}IúÒÀ;ɑ
ÙÝW¿å˜?	ˆÈo@
ΛzšOø@–€"û¿åsŸi½2ü¿äf>"z~¿åÿC!gÙ®¿×0T[¡çFOTHERsbg@ŒÁøÀ>-PowerLawNGC 1068?ïû"Ÿð©?M$n.w?C·u/lñ‰?M$n.w?ïÕ/²Ó¯ô?Œ/EQµÎ?uh&|ºêc?Œ/EQµÎ?ï±)Zí6z?yÁòZ{N?ƒµ©4ä-¨?yÁòZ{N?ïý&­zi?(€ÖÆ}¤?6ʓç3\ê?(€ÖÆ}¤?ïæŒê'8/?q3á)‹I·?isWÊQ%?q3á)‹I·?ïGn–÷?¯Áý‡o?—.IÍ%#?¯Áý‡o?1Bÿ??›eAmö?¥EŒí‡Ú	?›eAmö?ïƗ"4Í?u">ªëë?|´ov7Ï?u">ªëëAGN3FGL J0243.5+7119@`wL Õbž@$Ê· "À9h±Ä2ÊXÀ;r¨W¢~E?ڇKBƒ¶@}™èÉØ|@ãV€bc¿ÑÍ8[ÕØ~¿ä6Re¿âtÛ6ûrZ¿ã£üH‡Ð'AGNbll@¡Õ?|í'PowerLawS5 0238+711?ïý…³9Ô?/ø£à
DA?3×#غs~?/ø£à
DA?ïÅ@¯j?ÄÙ÷Í=u?}p_ÉG;é?ÄÙ÷Í=u?ïÜkØ/d?rº
¦—Æë?qÊϲU?rº
¦—Æë?ïÀ´†ëþ'?ZS°—êb?¥¼†'P¶?ZS°—êb?ïùJ¿þø?J¤ŠVn?J× Ý­ø?J¤ŠVn?îX=ÖWï?µ§½¯ß'?ªx"š?µ§½¯ß'?ï'"ИE?ŒJ²YB·A?‹~šÈjRß?ŒJ²YB·A?îÃðìM?".IÒLŒ¢?®óÀî§zô?".IÒLŒ¢AGN3FGL J0244.4-8224@r©óà7ÝÀ@ßL߬£bÀ:tÇR9‰À;Ă´zÆp¿ø•€Túe@¤ççÛF@n­ŸàÛx¿ëÚåÇÎü¿áwëøÕþ¿ä8_öhZ:¿ïýÀÈÐÇAGNbcu@~pÛߏG0PowerLawPMN J0251-8226?ï…T¥k+j?E¼¿ç˧?ŽªÖ¬]•?E¼¿ç˧?ïÑەpÑ?'k•«|Á?w5-ԏ'?'k•«|Á?îbÒç)U ?—š»PÐ1?©Òя"sþ?—š»PÐ1?ïÿsùª"?Ÿð2ӇX?€ÄtT6?Ÿð2ӇX?ï·çmf`?†5{Ûð5›?'ªÕ´?†5{Ûð5›?ïVò8¨NN?©ÂåQՕ?•!¸äþ:?©ÂåQՕ?í¨¨íÁÜP?¢ÚqS?²º¸'ñ~?¢ÚqS?ïónf‡jå?U¿kW•QÜ?Y#3e…6?U¿kW•QÜAGN3FGL J0244.8-5818@qf{à~íÀJ‰~¿ù³À:Õ¥¹cÀ;©ë-àãÛ?ғ&
ö4@
˞¤pb?û-í"Ti¿ç«/lìâ¿âˆÓƑv¿ÝE'"&?¬ùËÏ÷¥AGNbll@·ƒn—PowerLawRBS 0351?ïÿok«t?ú™îÀ:š?—pj…Ï?ú™îÀ:š?ïÌ0Ô¢óÏ?m¶Bl/?y畴x^?m¶Bl/?ïﴗ2n?LY.®q…?`KhíùÎ?LY.®q…?ïüê¯5ã?#âÊ
‡#?8ª‡¢tJ?#âÊ
‡#?ïÿͽsÐ?'éÉ6h7?æG«Žò?'éÉ6h7?ïJþªÚ"?°L€ÔÂ2Â?– *¨+J	?°L€ÔÂ2Â?ïé <Brä?l½ÆOÕ2?f_Ãÿ…œ?l½ÆOÕ2?ïê–äTö?\«sªÜ?eiâG?\«sªÜAGN3FGL J0245.4+2410@c7oŸËÀ?ȑ_8t¼À9)›«Â'
À;'ÇÖÃƔ?ðL"èÝy˜@JÃú@Mx@¦v pMp¿ä‡mÉqȿ稦&𯫿ꮇʅ¿ãä¼òAGNfsrq@¬ù	k¹ŒPowerLawB2 0242+23?ïÿ«úDTC?W)šè?vÏe·w?W)šè?ï¸('	F??¿‰{?õÛmà<p?¿‰{?ïÉ/­Ü`'?ph_¼0xë?{h)"MÞ¶?ph_¼0xë?è&?fÔ\ŽÐV?‡V…ü6zn?fÔ\ŽÐV?ïÿvNª¡Ã?ZÉr<Èo?6"†9ԑ?ZÉr<Èo?îþÛÅ/–é?­ºê? C­'r?­ºê?ï¨ZìNŒ?ƒn	þp…¼?…éDö«Í·?ƒn	þp…¼?íÞÏäY[f?ÂKfB?±	€ÛëJR?ÂKfBAGN3FGL J0245.9-4651@p]_Œ¨ÀN
dàTiÀ7š¹y2ñÅÀ;F{jÚin?øeZ‡àß~@imãÞ6W@ÊA€h¿âißW=ÿj¿åðxô'˜¿è? Ÿ»OU¿éåb¶6;AGNfsrq@t!˜ñ/LogParabolaPKS 0244-470?ïøЌ¹¦?Q؞⍺?O̾‹P"d?Q؞⍺?ï̀i¥h¸?š8VÜÑ??y?ËO§»¤?š8VÜÑ??ïC%SCv?åö´{?—›U—QE?åö´{?ïíøñ:aÈ?MB@¤åÔ?bÌ}oã?MB@¤åÔ?ïïR¤Ð?b,ƒjOùk?`­bî %?b,ƒjOùk?ï	údWý?µ˜/óHó ?žÀ³zEŠ\?µ˜/óHó ?ïLû‡€?'ú9s÷
?–`žü/?'ú9s÷
?ïàU¸™9"?f É\«€»?oªGƒ£–N?f É\«€»AGN3FGL J0248.5+4232@bÏÃøÀ.—VgÀ9û07EçÀ;Ö4O'åJ?ê¿7öûï@
'­õF=§@T̀K¿Ç¿éê7§ó5¿ØtKR¿êT™"·v5¿ïÿتrýPSRpsr@‰8®±Ä2ÊPowerLawPSR J0248+42?í²Ø
€Ç?µM×¾O>?²i?Þ¸É?µM×¾O>?癵Cˆ?ÇN©&×Á?ÐÍà•xïø?ÇN©&×Á?ìgQå>Í_?¥ÊE߸UÕ?¼ÅpÖ	•?¥ÊE߸UÕ?廐S8¦?¥jq†&¶}?ÔzˆßYŽ´?¥jq†&¶}?èŽDåõ¹?ÉÜá±¥ì?ÍÆìk¬)?ÉÜá±¥ì?Í㕼n?ÌފWçr?踇úå?ÌފWçr?ç'Ã⌺?´Ž
Q$Ê`?ÐÚx;Ðæ?´Ž
Q$Ê`?»¾G<ÄEY?—ÑÜüÑ¿~?ìˆ7gwU?—ÑÜüÑ¿~MIXED3FGL J0248.5+6022@a¶â—?ç*‹_Ö:›À7рuÜ%/À:rgᐩ0?ÿXŽ¤ž@ÊÈ.›@Î`=Wyd¿ãââ%­W¿ä"Vÿ¸¿êµDøØnl¿ïÿšFçPSRPSR@‡]ÌcñAPLExpCutoffPSR J0248+6021?¶ÒeÉû˜?ÁP_M\Õ?í%³F¥-?ÁP_M\Õ?¬säQ6?ÁÜVDQµø?î8Á¿o?ÁÜVDQµø?ÔBþAäÑÑ?³¬ä@-?åހß
—?³¬ä@-?¶µ'â~?–¥Rp¡cú?í)_]Ľp?–¥Rp¡cú?©¾oJ'T¿?¸¾ì#'ð?îd-Ÿd?¸¾ì#'ð?'̝§ñ ?ª£T'‰Ö?ïwћÀw?ª£T'‰Ö?È]~˜-Ö?¶'J©Õ"?éè YôŠx?¶'J©Õ"?‰Sê¬-[?zwô¦®±?¼GÛ?zwô¦®±PSR3FGL J0249.1+8438@_qåÿ£¹®@6my€žQÀ:
ˆÊ>}À;鯣ÇÀ$"Œ"xs@Ҕ%'_@,u?È¿ßù7r÷³¿èÞ X7¿Ñô²_õDK¿ã&rèÕÁéAGNbcu@ "RòäPowerLawNVSS J024948+843556?ïÿ°À¸Ó'?X91u:?Ïțír­?X91u:?ïݬ')©?ƒEþ1¶ÀÎ?qq*W!?ƒEþ1¶ÀÎ?ïïŸaÉb?\ÎK_ÌYº?`ã`à/,?\ÎK_ÌYº?ïÿÿLh0>—¦¿{=l>¯Ð3b>—¦¿{=l?ïÿ§"égž?²ˆçÿ4F?	ó]¿o?²ˆçÿ4F?ïamcÝ
?§l,$Öa?"ÒS¬Ò?§l,$Öa?ïí}Z­1?eyV;ù'?b'rê
þ¿?eyV;ù'?ïÿóºJr>â.Ê€ˆä>Ùڎ}Õl>â.Ê€ˆäAGN3FGL J0250.6+1713@cí€í )ÀB‡dàTiÀ9î&'d@òÀ;Ÿ_ý–™?뿸Àâo@v`Y‡?ÿ½±žÉj¿ê77ÙO¿èM^»Ðù¿Â2MD¬Wa¿ÖÞº_3AAGNfsrq@­mÄ2ÊXPowerLawNVSS J025037+171209?ïýÛÿWl?-c(X?1&þsò@Ô?-c(X?ï½%x=1?'ÈÁèQ¿d?€¶¡ß…®x?'ÈÁèQ¿d?ïÉÇèȒ?BVxœó»?{½c#l?BVxœó»?ï¯àí/Ã?dîäð÷Ñ?"Ä®h?dîäð÷Ñ?ïý¶±y×?6òÚM†‡´?2Ju+ôTú?6òÚM†‡´?î~îÀgŽ°?·:@\×?¨ø«.	?·:@\×?×k>ñ?Šsghµo?ˆ'Êáo×?Šsghµo?îىÜbA?ké¿)<?¢gb9ÛîÔ?ké¿)<AGN3FGL J0250.6+5630@a[¦?šIÃÀþ¬@:WÀÀ9ŒEÅ.îÀ;FÙõª;¨À{èP¶Ñ¹@z<Cþ¬?ÿØրÂ-¿Þ\†öÅ¿èVF3HµY¿Í›Ý '¡¿ÝEX"ƒÅAGNbcu@±ü'-PowerLawNVSS J025047+562935?ïýo¦ùJü?6ÔÆӞ![?4'É$@.@?6ÔÆӞ![?ï¼ëEw?',l€›á?€þE.J"³?',l€›á?ïÔÃíÞN?säͽA˜?už	d³€ò?säͽA˜?ïÿÿ°>¡`EBr\>nÖ%R>¡`EBr\?ïöú!¼	Ó?QZ)în8¿?R¼Eóٜ?QZ)în8¿?îfS¸?µVýÅmQ?§	Ÿ§Tâ?µVýÅmQ?ï¬}K|¢Š?…Õ!u"®X?"à­gÁq?…Õ!u"®X?ïÿõ:">áß
]¯fC>Ռ0}£˜Á>áß
]¯fCAGN3FGL J0251.1+2603@c=X@žUÁÀ=ƒ?ÀàÀ9´üÄâÀ;£XãÆäU?ó³	ªx¹û@Ä;dÚö@J3q¿Ôö¥»][¿ÞAç«ö=‰¿ç{"SÈeE¿ïÿƒ€¨†òPSRpsr@'-ØüPHPowerLawPSR J0251+26?ÚNu¦AÀ?Ώò{Ýò?âýXÅ,ß ?Ώò{Ýò?Ée°!àj?Êì«3
ã1?馓÷‡û%?Êì«3
ã1?ä‹ûBÎS?³¤WÔ €?×Úè	zcZ?³¤WÔ €?Ӄü%¢Ha?¢ÊDvñ[Ê?æ>í.ÛÏ?¢ÊDvñ[Ê?Ã¥¼¿°Ñç?ÃT–FE×?ëÐˆ?ÃT–FE×?µLVY
Ú»?Â2vž¿|?íVu4µiY?Â2vž¿|?È<ɉ1©?·Ñ»Ú°;ý?éðþ
³–?·Ñ»Ú°;ý?¡;œXþ®?šuƃ÷?îïŒFc«e?šuƃ÷MIXED3FGL J0251.5-5959@qu€?öÀI¤¨à^z	À:phŠ'¿À<FJg,_?Í퉊¼
@еd¦GÓ@QÇߨ½¿É2Å&\­w¿äÍÎZýÆ¿áåǥϦ¿ïÿ¤D1LAGNfsrq@'§ØüPHPowerLawPKS 0250-602?ïðg'^·›?lÇnâ€?_0Ý'éb?lÇnâ€?ï¼Î ó'C?"¥¬	yIš?€ÌW¿¬I?"¥¬	yIš?í׆eϝ?œìB.¸?±CÌÑ•?œìB.¸?ïû®ó¯ ?mN‰ù²Ô?‹ÁIóoø?mN‰ù²Ô?ïìæ0(ÅO?‰¶8sªjÏ?cϺ]ùv?‰¶8sªjÏ?îsüjãèa?´a¸'˜A?¨À9QÁyï?´a¸'˜A?ìá¾Â%²u?¦aí®4Tr?¸ò	ï@_Ú?¦aí®4Tr?ìMkÜOª@?¥,Ä¥©Þ?½"¡'®?¥,Ä¥©ÞAGN3FGL J0252.3+3830@boaŸÂ¨‡À2ˆw"^À:[àíìEÀ;Ò¡áf·Å¿ðvĖrs@'¶YÃÀµ@ø-Ÿ nË¿ä'†#+d¿ë¦Æƒ»š¿æ¡«;W™ð¿Ð–Æ\˜AGNfsrq@‰;Í5¨XPowerLawB2 0249+38?ïÿ"ª þ?¾É»
?ù–ôIï‹?¾É»
?ïÅD1!$?'/%Ú/?}]焻"x?'/%Ú/?ïØ?9Pٌ?iÍ,D1Ø?sàcm¹»?iÍ,D1Ø?ïÿàCˆQ.>åkÔ4•>ï¼·ÁÆIº>åkÔ4•?ïÿ9‹çÕ<?×­:øÀ ?Έ÷óµ?×­:øÀ ?ï.)ŒI¯?«ý¤MU2?š:Îq¸` ?«ý¤MU2?ï¦qè¿`l?'oÏ'g?†c…Úv¸×?'oÏ'g?ïýå'PjÀ?/"§ó ?0Öđ^X(?/"§ó AGN3FGL J0252.8-2218@j7ÿyÈCÀOŸÿå(
À7–>Õþ¤¶À;"™.9Ï?ø¨y @Ò'{™ÿE@ª"—(ü¿àÃý1…g¿ä£·F4m¿æà*R—… ¿çcò:<AGNfsrq@w[ËûµtLogParabolaPKS 0250-225?ïþ
-~Ø?2õ: :³B?/-'Ò¹be?2õ: :³B?ïÕªh7»?‡‹L'ãs¬?u*ËíÁ~?‡‹L'ãs¬?ïÛáxç"?ˆC3œÀ?Œ	žVƒ?ˆC3œÀ?ïþ%ËÒ¸?úê{¾à?-£?믟?úê{¾à?ïülJ‰™¥?BB>BRŒ$?<¬^¸ñ­?BB>BRŒ$?ïPXÈna?¬J	Иœ4?•ôæúÓùÅ?¬J	Иœ4?ï'c´ãՆ?—ÓsÚî"³?›‰áQ?—ÓsÚî"³?ïþGæôkL?&ÜÐô˜\?+'"ãÅ?&ÜÐô˜\AGN3FGL J0253.0-0125@fMþûôÀI'/`?Û¸À:Q¢xåÅÀ;ÄüÓ$Õ¢?ñŠ´(æþý@=s˜Óöã?ÿ.Î*L…?ïìóǞ Ñ¿"ÙsÌ+Š¿áê
ü™T¿æÅ&TŸáÕAGNbll@¢³îzáHPowerLawFBQS J0253-0124?ï³áU3ÒÚ?‡R×ðÆ#?ƒª¾¹õi?‡R×ðÆ#?àÙb[â h?ÏG´|Ç?ÞM;H;¿/?ÏG´|Ç?íÑàTéç:?£ÿ·¢òrt?±pýXBÒ²?£ÿ·¢òrt?ã"©×D?®Êh(‹X?Ù»ò¬QÏx?®Êh(‹X?ï'9%Eû?¢J•¡þ?›ÛcÖx¤?¢J•¡þ?ÔûÀ$-?ÑàijZo?å'ómþê?ÑàijZo?韼<²?¶F<ñÀ$²?Ɂ£:?¶F<ñÀ$²?Èu֗'?¯uGŠ2»?éâŠZ½6?¯uGŠ2»MIXED3FGL J0253.1-5438@q— /µÐÀKVK`P¢°À:iONóÀ<
Ñ@±¡¿Ëùî8W_b@½'ÐÄÿ@"°ŸðuÉ¿âps9ÕÜ¿æHŒ'0Tî¿æ"×½cÍ¿ìUaÀS0˜AGNfsrq@‡,Np:ûPowerLawPKS 0252-549?ïþÓ- 2v?$¿àŒ9)?"Í%D Ñ2?$¿àŒ9)?ïÒXß·'…?Œ´#+ÕÑ?vӐíŠ?Œ´#+ÕÑ?ï»Eœ¨}ô?v«=s†?.˜ãöèà?v«=s†?ïüŒ—l\Ž?# 1aHb?;›Dp|?# 1aHb?ïÿOƒn~?åßRA¶?šÕ{?åßRA¶?ïpK¤eœß?£'ä$?'ö‹z+œ?£'ä$?ïՃ9RS?z®ä]I?u>cf¤s@?z®ä]I?ïàÓeòí?`ߗ¨DV˜?o,›i*«?`ߗ¨DV˜AGN3FGL J0253.5+3216@bÞ>ߤ?æÀ7๿©Î›À9±€•Ó;À;*,ú4¿ø4w
þp@áܼ.@k@?
W¿å,¶Á6…g¿â
2Ì
¾¿äï«õøÑI¿"ÁjÕsAGNbcu@£,°|"µÝPowerLawMG3 J025334+3217?ïÿÁäô8?ÜÎO¨«Ê>ÿ—*R~?ÜÎO¨«Ê?ïÓ¹ù¾ûÜ?Š…À¶Îd¦?v#5Ï¥±?Š…À¶Îd¦?ïæú6E?fAŸ¹l"i?ií»ü|?fAŸ¹l"i?ïÿÿÞ¶Èî>iÝöøQ>p¿C•Œû!>iÝöøQ?ïÿœfí8Â?3mž8:?æTA§ù?3mž8:?ï[©ßëk&?©Q6ãÈ»?"ŠÄº5?©Q6ãÈ»?ïÏpqta?<RæL?xGþµg×[?<RæL?ïÿþñô4×>¥C–Sý}> ä¾Ú©¿æ>¥C–Sý}AGN3FGL J0253.8+5104@a¸ ٔ[ÀcßÎ\DÀ8´w⏬±À;7ÞUõÖ?ÛJg@C˟¦#@Z9€ª4q¿çEZB¡¿ç¥¼'—ó¿ç^†7Ó¿æÎæ‡ÞÜAGNfsrq@'Éj%™íPowerLawNVSS J025357+510256?ïÿ{ëUEy?àÊ¢jÜÝ?'¸®^Ï?àÊ¢jÜÝ?ï8}¨ï?ŸG'åXp?ˆ±à§(?ŸG'åXp?ïÖ)ѓ9?u1߶]nv?t÷k˜»Â?u1߶]nv?ïÓOç&ž?V§Fî‡û?vwXy?V§Fî‡û?ïý6—/¡?7ä¡Õ€Õ?7FJ'ŠÂ?7ä¡Õ€Õ?înùÕ:ý?¸cœiè?®©`›7?¸cœiè?ð•ÝU?‡šO»ÃÔÅ?‰›ä×~®?‡šO»ÃÔÅ?Â$I®?øQNÀò?¦EóàO ?øQNÀòAGN3FGL J0255.8+0532@eFð¸,,ÀFÌëÿ—û4À:L‰°îIõÀ;£´©^3?Ñ¿tâ!•@
€Ý°ŸÅƒ@Ž¹?|AÅ¿Úkk9É¿äÁw:ß@¿Úo/@h¿æ÷–<ËkAGNbcu@¤àì"h	ÕPowerLawPMN J0255+0533?ïÿzwуý?£"çì?±"¢79?£"çì?ïѶbkôµ?‡(˜ûdó?w$ÎÇEõ¾?‡(˜ûdó?ïßÿ‡ùÎ?kÉ)'?p}€L9?kÉ)'?ï¹µWT—?`{J "ð?'ªÜÒA?`{J "ð?ïþʾT¹ì?"›•F"º?#T«6"ƒ?"›•F"º?îљížËÕ?³b݂U?¢æa$[t³?³b݂U?ïµ@v'?"YƒÛÀ{H?'¯ÿèP1?"YƒÛÀ{H?î
Û¹œ?˜ïMJù‡ó?¯"N°þjH?˜ïMJù‡óAGN3FGL J0256.3+0335@e‡y¿ß~€ÀG{íÊ»{À:;ëß·‹À;©ãiÇC÷¿÷YeqžÓÀ@
|=&|?þVE^®â¿ÙÉ÷9 Ìÿå€øiø[
¿ßaœ;¤4¿Û%¸«6AGNbcu@²³¶E¡ËPowerLawPKS B0253+033?ïÿô˜
?ŸK‹ž?bº'±?ŸK‹ž?ïÕLJ¾zÏ?û€</Ä?u<*a€3?û€</Ä?ïֆÿ…~&?z>ßͧ0?t¼€Tq?z>ßͧ0?ïÿäÅø>án)ÍÒð4>ëÿÿÞÂ*>án)ÍÒð4?ïÿtu%y•?J;bs—ƒ?qX&>l?J;bs—ƒ?ï&¼pšX?´UEr·â?›(qêý/-?´UEr·â?ïÐ\¶†±­?|ÏÜmÉó?wѤǥé…?|ÏÜmÉó?ïýú"µ%€?+k³qÏÙ?0.ìÓ°Ž?+k³qÏÙAGN3FGL J0257.8-1216@hsÿ¬*ÀLr 6×-À:¶'Τ=À;ߎ¿K
?ßғ»‰-'@WðK'	…@Òýßê5é¿Þfé=¿ç;æqÓEÒ¿è\+´d1¿è71¹¥A‡AGNfsrq@…Ù§»/ìWPowerLawPMN J0257-1211?ïÿڈC¨C>òÔ]•õ7>ò»Þ¡¼¸>òÔ]•õ7?ïԑ¯6Ü-?ŠÉ÷*O|?u·(P¤-×?ŠÉ÷*O|?ïÑ¡á«?ro?™-õ?wr¯zŽ?ro?™-õ?ïòú!Þeë?<¶—(n%?Z¼ûY÷?<¶—(n%?ïÿÅV¥—î?°0gW±>ýT£èÈX?°0gW±?ï%?YdÔ?²~˜å©7}?›\x
ô-'?²~˜å©7}?ïaÀ‡Íœß?¸fœÜ?"Çï
+œ?¸fœÜ?ï·}Ü%?oÒGZéw×?' ¹|ñ"Ä?oÒGZéw×AGN3FGL J0258.0+2030@cßdÀßXÁÀ@¬‹ŸÛÒúÀ9úá:B.À;{E	õLH¿õq.÷iÐ@'Ý/p…ú@!VÇE¤¿î[r:"U?Û¶æˆñ½¿ä]}«ô²¿Í.–Ì	ÙHAGNbll@ªdú¹õY´PowerLawMG3 J025805+2029?ïÿtǏè?Õ#©À|?g•ÖÌà$?Õ#©À|?ïÓìv9‡?‹—Ûk…÷?v	¹,Õø¥?‹—Ûk…÷?ïÛ¤-3Y?v?Õøÿ?r-øeö·©?v?Õøÿ?ïÿë|T(:>Ýɔ›ZE_>䃛Ç[>Ýɔ›ZE_?ïÿI^LF?G1ۘ
?ÔF}ý‡û?G1ۘ
?ï"Œ#0Ô?²¿XÊ5\?›¿nvr{‡?²¿XÊ5\?ïÒ¦1œI?|¿XC¼?v¬ç%|ßú?|¿XC¼?ïþ£ÓM?(&tqõ(?%ύ3àe?(&tqõ(AGN3FGL J0259.5+0746@e$»%_5ÀE§ÒàD²À9E<æÀ"À;qkI$6@?ÙzAµ,>@ÇâöYã÷@²v BÀš¿â9˜/¿¾Ð¿å?U÷i¿ßK|‹ýàÒ¿ìfçsI×AGNfsrq@"Ø4!-wPowerLawPKS 0256+075?ïþv!3EA?#"=µ©Š§?(ëÊbÑ£?#"=µ©Š§?ï׍Ȩ?‡HP¯M"?t9}¼þs?‡HP¯M"?ï|+wیa?‹½`?zý¯;ï?‹½`?ïõhâ9?6°BÄ1å?U.;©M?6°BÄ1å?ïýØîn28?1f\ïkƒ#?18‹ªÔð\?1f\ïkƒ#?ï!4v1é?±M0¢pi?›Ùq9ÂÞ%?±M0¢pi?ïY%con«?""A‰äÐ?"ÛS—9"?""A‰äÐ?ïÕP¥¥w?f2ݶ?uW­h¾èV?f2ݶAGN3FGL J0301.4-1652@i~à°¯`ÀM"€ŸÍAÀ:Yx°"À;ßÿê0Šâ?îöŠâáP@*³In@4`BŠê?îÊ«ÖÊ+¿â²W¿Úv¿ä¼G_°¿è$å?èÖÌAGNbcu@–ž)xÔýôPowerLawPMN J0301-1652?ïôíìÆ×?Y²Þõ{e$?WÔ#Ü:Â`?Y²Þõ{e$?ï|ì9F.?—'ùÃú?bxÞ²<?—'ùÃú?ïcǓZ˜Û?‰œÃð…8º?"‡
…z›?‰œÃð…8º?î̂¥h?Žôkxÿ-8?¯"7Ó÷{‡?Žôkxÿ-8?ïÛÓ¾Œç?z]Æ:|Ÿ®?r ÑýP]?z]Æ:|Ÿ®?í À)®Ù?¸iD«ð?¶ÿiþD•»?¸iD«ð?í…šU£˜?ª¨¨¸íÞ?·ÃÓ,	Â?ª¨¨¸íÞ?ç"w1uÿó?²ø"œ;?Ðם?²ø"œ;AGN3FGL J0301.8-7157@r ÿâ£ÏÀDߏÿ¼ä!À9©&Á½¥À;ìAVâdå¿ýÛZY<Ý+@ѾÎ\nì@ -à
q¿æþ¶"Ç¿ê¿çd…'*W¿é9ð¸Jšê¿ïþ×;ï"AGNbcu@yb/¢ðZqPowerLawPKS 0301-721?ïþšÙEè(?$$J ›-–?&Rnc`qÛ?$$J ›-–?ïÚúwéD?‡q9Í,ùE?r'Ä3¬Åè?‡q9Í,ùE?ï¯>QÒä?sh}aÿ?"0k—ý‡?sh}aÿ?ïÿõ†Tmk>ÐjÏñZ»´>Ôóþñ­Ò>ÐjÏñZ»´?ïÿ%t®¨Ÿ?ç{QrQÌ?Qf!a—|?ç{QrQÌ?ï1ff*E=?³«Íwhþ?™Ó38ÿŠk?³«Íwhþ?ï¾hh5§?ƒf¦‰X?€eûíÙ°3?ƒf¦‰X?ïÿ2µp ?{W8ä?±§	s6?{W8äAGN3FGL J0301.8-2721@k =ÀTïFÀN‹_ !¸À:ÃhÍJ¡À<îл?Í°¶h)@
`+¾ß@CA¿½ð'?ßóä²áX¿Õ¡ Á"–û¿çšS|:p¿ãºØ0AGNbcu@›8<ÚQPowerLawNVSS J030158-272754?ïÚ½AsÏ?¤ÿîi(k?r¡|ÿ'l^?¤ÿîi(k?ïÂ@©'	?‰uCà«?~ßó$C™?‰uCà«?ï" =ø‰?"}"ÞÒfr?œ[«ôÑRâ?"}"ÞÒfr?ï<‡3ª@?ØÎôÖgf?˜oü?ØÎôÖgf?ï¹/a ¬?‹ïÁ•øT"?´'Ž7?‹ïÁ•øT"?íg‹ƒÆƒ?»Úrµä?´Ã£ß©Úk?»Úrµä?íÀ´¾Á¤Ù?¥îd[&ö?±úZ
ÎÀ6?¥îd[&ö?åð¿ÈNÛ'?½à!µ©¼õ?Ô€obI²?½à!µ©¼õAGN3FGL J0302.0+5335@aµt!-wÀÎëÿÂîRÀ9±ôafLÀ;RN©±>Ò¿ÕáVՂ[˜@­Sk7¦@'€L–‡¿Ó^(²Ú:ý¿çl*³e{¿ê½·õ¾ø¿Ö—I³'_@AGNbcu@"òyÀëíúPowerLawGB6 J0302+5331?ïüÊ«àC!?@Á*½MêÎ?9ª¡È6[f?@Á*½MêÎ?ï´ê-Û°?'h'"¢xX?'üs);ç?'h'"¢xX?ïŽt4ZO­?…j¡ÑÉr?ŒbòâŒÜÛ?…j¡ÑÉr?ïþbÚHi?Ù­ªâÏ4?)ÒYZG,u?Ù­ªâÏ4?ïî‡^GwÓ?cãäßDËð?ax¡¼§µl?cãäßDËð?ît:(è#?¶í`îÿ½ë?¨¼]p¡èC?¶í`îÿ½ë?îs\`œË?Ÿ
çÞO?¨Ê9ÿ¾Q?Ÿ
çÞO?ïêHu\ÿ?`ºˆ›%P?e·Š‰Èù~?`ºˆ›%PAGN3FGL J0302.5-7915@r|>KZÀAýVÿÁßÀ9æêºô]À;¾˜Ã°ÄYÀÆã<û³ë@:Æ¥k_@R_žK/¿âß
e²ü¿è†BPÿÄ=¿Ùv?/Y¤¿ëæŠx
õõAGNfsrq@†"¡–R½<PowerLawPMN J0303-7914?ïÿ>"eR??KC©:ˆ?-v­# ‰?KC©:ˆ?ïÐMè7®º?¼]ðŸZ'?wÙížÄ?¼]ðŸZ'?ïÅñy²üö?sùï/Ñ;‹?}C+Pù0?sùï/Ñ;‹?ïÿþ4ù±Ý>¯$Bâè•Y>¬´¢óÖ¿ÿ>¯$Bâè•Y?ïÿ®HI½0?ùË÷ñå?mí59W`?ùË÷ñå?ïsSט'Ã?£žä:t?'•…7ٛ?£žä:t?ïÚÁü~,?~™ºê·ÅZ?rŸ¤ÑV?~™ºê·ÅZ?ïÿæ!²'I>êkÿNª>éކ/Dì7>êkÿNªAGN3FGL J0303.0+3150@c"CŸý`éÀ79՟Ú%{À:1æÒ1œÀ;ª²²oSu?ét4'®ÃÍ@
š{'pÖ,@…¿rÇ¿Ú¹éï¿åsÍl¯Ö¿Ù¾Uà *‡¿ïÿÜBê}AGNbcu@'<Âø7´¢PowerLawB2 0259+31?ïñˆõ©Ý?dò<…-Ý!?]Ôî%*e"?dò<…-Ý!?íôž'6Yê?¬"tRΉ.?°[xþª?¬"tRΉ.?í"ڐî¢?¡.Ó
iÜ?³Ù+}ºÉs?¡.Ó
iÜ?ë˂¡ý¸Ÿ?›ÖtÜÄé3?ÀÑõx	'?›ÖtÜÄé3?[½k?"m•ÚE?‡)7a	=?"m•ÚE?âäp‰nÂð?ÐÀÙÆÒ¯?Ú7í"z ?ÐÀÙÆÒ¯?ê'‡—IÄ?±ƒ¬§¦=:?Çc¡á¢Øï?±ƒ¬§¦=:?ßÝ^¦²v?½úÉ
Í?àP¬¸&Å?½úÉ
ÍMIXED3FGL J0303.4-2407@jÔ5 ÝDÀN‹`òËÀ7qJ½"sæÀ:¥C'&Ò¿ÏÓXî@ÞõCc'?þ±Zá"Z¿Ø,ôˆ¿àÉÇ{C)¿Üs,aK¹¿Ým8<²béAGNBLL@"\£S&PowerLawPKS 0301-243?ïâÉ|þ"?­ƒ¹9pYÇ?m6ƒø,û?­ƒ¹9pYÇ?ïÓ\PR?Ž[-D©¿?v~pÞæ[
?Ž[-D©¿?ï¹5
RùÍ?†ÇÂ3Ý Y?²¼µ`¯?†ÇÂ3Ý Y?ïÿýÀyq>¨ÓŠ2·O>±üðSÙ->¨ÓŠ2·O?ïþÅ·sŽ?%óAKâU?#¤Š±vÛ?%óAKâU?ï:"€H»?±¦ºc›Ð?˜­œ)°´?±¦ºc›Ð?ïå'K¹´9?| ¨ÁQ?jn´z…×?| ¨ÁQ?ïÿüÓ¶Ý>¼p7£ÐãM>¹a¡Â%ù>¼p7£ÐãMAGN3FGL J0303.6+4716@b ŸDÔEÀ#¶î#;nÀ8SJM++þÀ;N"šVWû?çÂ6oÂts@å-oÏƧ@D¦€1釿㞎ŸÚ?@¿ä¯àWæh¿äú"â?¿ããœl²°ÂAGNbll@Š&Ž¾ß¤@PowerLaw4C +47.08?ïÿ<#za#?#HÀìºÿ?{Ä!}\?#HÀìºÿ?ï¼ÖîÜ?Ž¿ë-"?€û
?Ñ~œ?Ž¿ë-"?ïٗ'›Ç¿?rÐìÔ>-?s4lŽ<Ñ?rÐìÔ>-?ï÷Yu!?4ÝIt ¹ã?QõM]w¥?4ÝIt ¹ã?ïýâÂ5!Ó?1»FÓXöÒ?0éí%GYs?1»FÓXöÒ?€‰Žp?°cuÔ?¤7×øC?°cuÔ?ï?½ë2"{?'§¼g¼â%?˜B ŒÈ"?'§¼g¼â%?ïß¾	C(Q?anz¯%M?p ûa+‡L?anz¯%MAGN3FGL J0303.7-6211@qƒÄßÎ1QÀHZ$™ù;À9!ý¥²¬À;´Ñ¤¢â?絶"ï̵@ëxˆ§Ú@®ZÀr¿ä8ÚSÀhÞ¿çVbÔ¥M¿åD'â7†¿ê€?(ðö3AGNfsrq@†Ô|í'hsPowerLawPKS 0302-623?ïþXkYß?&h$«'Úé?*yN)N)¬?&h$«'Úé?ïƎ©?mÃ?ŒZ6@ÿ…¤?|¸«RŠ®ž?ŒZ6@ÿ…¤?ïÃoð3?t:{O¤Q‡?~HuõX'Ñ?t:{O¤Q‡?ï'õÄ?i4¦ý¼£?‹B¸ÿhêö?i4¦ý¼£?ïþ³¨t¹÷?*"¾ _I5?$ÅwÖF—?*"¾ _I5?çfÏ?´¸ßG =þ?¦Ôá‡-¬?´¸ßG =þ?}ß¡2?Œ{ð@ŽHT?Œ• "¨w?Œ{ð@ŽHT?íxç÷\ï?™éVƒ?´8ÀB©1?™éVƒAGN3FGL J0304.3-2836@kõ¤€èȬÀNWþKZÀ:òº.d—YÀ;æÃ$º?ðíÇ¢@gËOKE?ù½AÑ6>¿ï»¹/7Å¿Ý㔏nm?톣Ùʝ¿ß…±">jAGNbll@¹Ó¨ -àPowerLawRBS 0385?ïúdÚµ?@ÕߧLS?Fl—8F?@ÕߧLS?ï©ý°Mé?¡&fÙN?…€"ýè'?¡&fÙN?ïrsÏIm¡?‰¨<Åd?ô?'±†óé?‰¨<Åd?ô?ï«ù= Ð?~¼3Gè?… Ÿ‰¿ÿ?~¼3Gè?ïû<Z_ƒ/?@ދ2wÐ?C–—ðÅÐ?@ދ2wÐ?îQ'ÿ?¼Î0O(1L?®ïŠé
?¼Î0O(1L?ïo 
*z?•ûÔ&|NW?ž2ü¢âÊ?•ûÔ&|NW?ïˆú"j½?›{¥Z'M?ùAhãÀÆ?›{¥Z'MAGN3FGL J0304.9+6817@`Ù´ßݵ@!*ŸæºµÀ8±ÕORM«À;PgžtÊ­¿àiÐu›/@‰7jöC@Á`)áP¿é]£G©s¿ç5¬âC#
¿éÞ6%DÌÒ¿ãQj͘ AGNbcu@rx':)ÇzPowerLawTXS 0259+681?ïûþp³ÇB?@ÕÙ;Óò?@<Âïws?@ÕÙ;Óò?ïÒ4öàO>?/ëL¥…?vå"vkE	?/ëL¥…?ïÐÿŒh?Š.0€U™È?Œ>KÍÛV?Š.0€U™È?ïøMø—'?@®e~YoŸ?NÈ‹-tÀ?@®e~YoŸ?ïä¿š'Æ?p"ìLe§ƒ?kø@A±I½?p"ìLe§ƒ?îÀš*ýÉ^?´ð²áv?£ö]Nkœ&?´ð²áv?î{9xû? üÑ^mMÕ?¨OÌeܙB? üÑ^mMÕ?ïe9HÝ$Å?‹]˜îk0?"XÖÝ|/l?‹]˜îk0AGN3FGL J0305.2-1607@i
l <K
ÀL'BàO`À:Š:¶µ3SÀ;Æjd!èˆ?ç·Uðêc@
x¯¸k?û!Û­?ïºSzÍR¿éévÉ¿º6'äÌ¿»Téj¬
#AGNbcu@¸gÇl‹C–PowerLawPKS 0302-16?ïÿZ1`Š?'zDNm?¹Òø¾yT?'zDNm?ïÆjZðD)?'pùô?†?|ÊÒp€"µ?'pùô?†?ïÓËW	"Â?tF°þ¹þš?vTlÏCB?tF°þ¹þš?ïåµwß?UrJk½?jJâ6¡hÏ?UrJk½?ïþ涔x?#FÃ<%q®?!"™Gîºá?#FÃ<%q®?ï9æÓUŸf?ª»®Y~¨P?˜Ã%•L:?ª»®Y~¨P?ï·rÜQ¶<?jÅ {?'#Hð	îæ?jÅ {?ï·ì|%ч?tÈq`!ù.?'àósøD?tÈq`!ù.AGN3FGL J0308.0+7442@`w¿Â"O@,o[Ao6À8ó¸ÒDÀ;Ý@ï´Xb@H² y@\z-m¡n?èh°n$ÿF?ã±i¸"A¿Ò:…ÚAvå¿ç[ooyŠ…¿ïÿñ­µcPSRPSR@½•*™1PLExpCutoffPSR J0307+7443?Oá×·p|?cÀ¨7}Uý?ïø9ǙS›?cÀ¨7}Uý?±·{/_äÎ?Å(tpó¼?íÉ™ø††?Å(tpó¼?°\òˆ€ê?£3k¸ñß½?íôa®Æ§o?£3k¸ñß½?y™1ªá?bo*–0u?ïÌ͜'¬Ì?bo*–0u?f›áÕj§?{ñì÷!¥?ïédï))U?{ñì÷!¥?šê™=2£\?²uŠ@—<?ï(«5ßq%?²uŠ@—<?¥ԌáYµ?Ÿ{Œo7æä?î®â·MgE?Ÿ{Œo7æä?DÎ3ÉԄ?83‰tY2D?ïúÌrðô†?83‰tY2DPSR3FGL J0308.6+0408@eÜ:Ã.¾ÀF;à0VàÀ9¾Î?""ÆÀ;#†Ö?ÛÏÐÄsq@ðE®_ú@'‹ßǦG?ïðBÐ+ž¿ê,²€=¿Ì¦†iр¿â¢æ1ð
AGNrdg@žpµY³Ð}PowerLawNGC 1218?ïÿ!³%~6?ˆÐ‡l?ɖ÷"Œn?ˆÐ‡l?ïËY'J?Œ¸Œfً?zSž»«^?Œ¸Œfً?ïÞ_%W)?kVÖpÐz¿?pÐm{c¦?kVÖpÐz¿?ïÃH²©é|?aÕդפ8?~[¦'N\?aÕդפ8?ïþO'ýÂZ?/M§†è8"?+
€¬1>?/M§†è8"?îíì¯7²ì?´à˜1&Íü?¡!5"Ñ>?´à˜1&Íü?ïÄÚ&Éå´?~ÉPñÖ
Õ?}'ì^z?~ÉPñÖ
Õ?ï)žnŒòå?…Y»É:?šÌ2*òt?…Y»É:AGN3FGL J0309.0+1029@e%F?ÀCێÀ!ßÀ8kÖÛCˆÀ;-T®­ýÕ?öÝ7ì*‹@™»þHp?ÿã»(Š¸¿à.–PŽã³¿â]ÎUŸ*¿æžƒ8â¨4¿ä
(|Bh'AGNfsrq@†cL~($LogParabolaPKS 0306+102?ïþ¾{?*Q?!DPNÅ:Z?$M¨''É?!DPNÅ:Z?ïÐ&èvþ?Ž«K6£ïÎ?wì‹ìvM?Ž«K6£ïÎ?›º8Ô?"²£‰e! ?ŠPY/?"²£‰e! ?ïüæäÑõ?$jÊÕúéƒ?8Èát)Ü?$jÊÕúéƒ?ïýM
Q?<9$¥"žÍ?7–KHí?<9$¥"žÍ?ïE¼iæ½?±+^PùJ?—HoÊ,"b?±+^PùJ?ïUHlˆòá?'ó\$Ø?•Vòiº9ê?'ó\$Ø?ïû²Ù0³Q?:¥î½¶È?A4š¡žÛ?:¥î½¶ÈAGN3FGL J0309.5-0749@gš·?1n7ÀJWÿ›V2À:åsŒ¿—À;¬Æ8^_?Ϥ'౟ä@Lªhö‹?þöý?†RÀ¿Õ}¥kΞù¿âéC¡¦"?µá݈ºVÜ¿èœ)×È\AGNbll@§"Éûçl‹PowerLawNVSS J030943-074427?ïý*pŸ'ð?:ôùM5
½?6¬|Ƶ;£?:ôùM5
½?ïÓô@ÚÖ?…0*@û…¸?vߟV¬¾?…0*@û…¸?pž3Ú?'Ìš?ÿ&?€›ØƒÒAˆ?'Ìš?ÿ&?ïÖؘ¡»Á?^ˆÆšþþ?t"³"U+½?^ˆÆšþþ?ï÷Ùtë?WØtÖU´€?QÃÔ\»?WØtÖU´€?îøæ»áB%?´£©ã{s? q"C£«²?´£©ã{s?ïsUµi-ì?'ñ¿#?'•IKû
‹?'ñ¿#?ïdkSØf«?ema6?"r•ƒŽ›?ema6AGN3FGL J0309.9-6057@qa¦`ɊÀHyðßьOÀ8Ÿ' <¶À;¸éÀùZ?èªXðeÞ@׌yËs@_žŸ½Êü¿â!©¢?h¿çÚñA
¿ä;Ýòö}¿èb]{AGNfsrq@‡8Úþ§±PowerLawPKS 0308-611?ïÿÜr‡1?+\eÃÒ,Ž?äjÄ5Ö?+\eÃÒ,Ž?ïˤ%¹¢ù?è˜±òhÙ?z-íâ/x?è˜±òhÙ?ïÊnjϏR?€<Ž5r?zœ9¯•®¤?€<Ž5r?ïñB+¸Yg?AÝ0'Ã|Ô?]{¨¢‹¿?AÝ0'Ã|Ô?ïÿ(S0?!•4ã="ß?íîæÁ*X?!•4ã="ß?ï.k =ç?±'IcŒœ?š2›ö¥•$?±'IcŒœ?ï"Ê2úºW?ˆ‰ˆáW̯?‹
sDÁ7?ˆ‰ˆáW̯?ïËúævÓ,?jä sÆ?zŒÐõË?jä sÆAGN3FGL J0310.4-5015@py'ß֔ÍÀKr<à[À:3maÚÀ;»€šŸS?ìêjûݗ±@õ;Øbç?üÈ>Ï¿éFчƒ?Ö[4®³\¿ÒÑe™žy¿Ö|뗬ô.AGNbcu@±‰}žƒä&PowerLaw1RXS J031036.0-501615?ïþ§Û{¼9?#Pf¸,j	?%'KSžç?#Pf¸,j	?ïЍ‡¦?Šý`oTÂ<?w¹tÆ"ø?Šý`oTÂ<?ïӉ»Ûõ?zvºÖµÄ?v;"'AQo?zvºÖµÄ?ïÐöcZSš?U‹™	Q'†?w"ÎCÿ5?U‹™	Q'†?ïþ¢íÖ1Ð?#zvl§?%Ñ!Ôƈ?#zvl§?ïxp\¼ø?³/4¤a«?ŸpñëÑ[
?³/4¤a«?ï³÷(ôs?‡Tå"ày?ƒ5̂–?‡Tå"ày?ïqBWµÁ?z£~٘?'Ü7»èÚ?z£~٘AGN3FGL J0310.8+3814@bÝF€"À0ñà18‡À9›á·?œÎÀ;š­•Ïà~¿ø´Ô2œµ@cÏÞ$8@c x›r¿èÖÚJlh¿èBxŸñCò¿ÖŽ*ľz=¿ékë-ŠýŸAGNfsrq@Œyj³g ùPowerLawB3 0307+380?ïÿŽ½¿àø?	ý¡¶÷ÿ?P—œ,ì¦?	ý¡¶÷ÿ?ïÏMCÄ?ˆ˜úè]ä?xY8x:ýï?ˆ˜úè]ä?ïÙÇ¥NY?xê	J`ß.?sv‹ßÑ?xê	J`ß.?ïÿøh†ý
>ÃN¼÷nÙÐ>Î^#À¥ë>ÃN¼÷nÙÐ?ïÿ'A‹—?4֍¨ïà?o¦G‡"ñ?4֍¨ïà?ï/@ª•z?©;'æ|`?šê´<¨À?©;'æ|`?ïњ8Ñ
?£*xäÂ1?w2ùí6b´?£*xäÂ1?ïÿº0¤è?Âel¦ô?sèÛq?Âel¦ôAGN3FGL J0312.7+0133@fP†þ÷ÂDÀFÁÿÑÀ9$5Ý1žÞÀ;×xø?ÒSDܺ@'èá'*@B¦@#¿áëŸè,œ¿ä
ÔÝp¿ãÁ&~¢zò¿ãÓgTmãAGNfsrq@sa»ûPowerLawPKS 0310+013?ïÿÕY¨Ô>ïíÛhÍ>õSEæuF>ïíÛhÍ?ïÏqøjàI?'KÊé#ÃÊ?xG¾á/»?'KÊé#ÃÊ?ïí³UòÈ?Ze"àv'£?bLªk˜?Ze"àv'£?ïÿ4ƒjX8?Üß°9¼?ošƒâr?Üß°9¼?ïÿÐ`¼>›>óÀVö‹è>÷ϗq>óÀVö‹è?ïD³[À"Î?®]»-NS?—i"ŽÚÞ9?®]»-NS?ïÑ#¸ä/?|KÊPí?wn#uÛ6c?|KÊPí?ïýo…&£‹?(˜BJY?4ƒÕ¯7y?(˜BJYAGN3FGL J0312.7+3613@ce`A‰7À2mêÀӚFÀ9ö"ö¥
kÀ;œ'«hÎö¿¡](þlR@Pà$ÃXÛ@E"…á׿ä'
Õ#»ú¿åàÆ£V˃¿âÑz­Ž!¿ãRt‡ï×AGNbll@™3"g8~PowerLawV Zw 326?ïÿ€~?¡?%GÂGb?àf»;Ó?%GÂGb?ïâìvÜ?'‡@Ôño?~.‰ÄO%Þ?'‡@Ôño?ïï'ŸM?`
Â''?`ômãòe?`
Â''?ïöU¦iz‡?8ÑS"ö|Ú?ST³[Å¢.?8ÑS"ö|Ú?ïþ××ý?(×ÌýZæ?"'H~X?(×ÌýZæ?ï
"ëè?©'j°«?ž]»¢'÷?©'j°«?ïʹ¨"î›?'¾–™V?z£+º(:s?'¾–™V?ï¥K6©ñ?u-»5³Þš?†­:õÅ¢?u-»5³ÞšAGN3FGL J0314.3-5103@p…B 6mÀJýJ 7BŒÀ9˜0P)ãÿÀ;ÝÕC"Ó‡?Û«Qß¾
@oŒhC5@3üu¼¿æô ¦ò%U¿ãžlO'ì¿æKr7#¿Ù©©1£LAGNbll@ˆ‰3×ÛõPowerLawPMN J0314-5104?ïü펹@Ô??‰&™~G?8"Šâg±??‰&™~G?ïÊ>lnµ?Ž":}ðß?zàÉܒõ‰?Ž":}ðß?ïÀÉw
?tS;–΃?›DdÁõ%?tS;–΃?﬷ìÉu?iö>Ä䆊?"ÒÍ¢¾9?iö>Ä䆊?ïäõE/?s@š<ÀDe?k
ºÁ£ù?s@š<ÀDe?î^ŠrgÚ
?¶¾,¨­ó>?ªXÜñû3?¶¾,¨­ó>?îy¨Îssž? ê1Vw —?¨es\{!? ê1Vw —?ì\«~ÀǨ?©ÎA?½¤	ù¾?©ÎAAGN3FGL J0315.5-1026@h7¹ÀëíúÀJ=Ÿ¿™À:@¬˜yßÀ;¸­7Ü`À«Ðo¼@ÔÓêÎ?"@GÑ?Î!6¿æfݲMD¬¿æ™¡Ž|ýN¿×"U0¤¿ê™ñùWlAGNfsrq@=°O‹YPowerLawPKS 0313-107?ïÿÁÛú^£? zC/>ÿ
\ÌÄ? zC/?ïÙ{Ô·§Í?‡Q;ĶJ?sB˜}mÊ?‡Q;ĶJ?ïß$\o†d?fî†¢Ñ9?pmÑͼ-½?fî†¢Ñ9?ïÿÿ4†¢ú>•$¤ø¨³>™nùêÔ>•$¤ø¨³?ïÿäëì;—>òûˆ€e>ë'O ó >òûˆ€e?ïCØ.Õ«n?³Cy]Jm?—"ú-á˜??³Cy]Jm?ïáôYX¶Ð?wb‡l?n¦Öß^?wb‡l?ïÿøž6â?>θ)¨œ+š>͆'‹ïY>θ)¨œ+šAGN3FGL J0316.1+0904@eƒ  ôØÀCÌ¥ 8LÀ8aCRe'¢À:õÍêÙþ?áØZx2
@°¡€mΐ?þ©; jM?ßÄèÅÚGè¿âÖ¶ÓÕÞ¿ÜR­Ÿ¾`¿×ïNBßAGNbll@¢¬!aä÷fPowerLawGB6 J0316+0904?ïÿªrYä£?‡ëÊÙÂ2?cg‹NpÁ?‡ëÊÙÂ2?ïØmoð†?²
M9°W?sÉ1E÷øÌ?²
M9°W?ï×°õš(?vSZY£?t'…LÔó¤?vSZY£?ïæaò?O®)]AZ°?iž
¦—"	?O®)]AZ°?ïÿuxt}M?
üù?1r	?Pê[Ýb?
üù?1r	?ïN4=@ʘ?¤ëf0"¯?–9xQu
?¤ëf0"¯?ïÍØGï>?'9aVL?yþJ*i?'9aVL?ïâ½,¤?vèÔ1öhA?ˆ¹[ªÜ?vèÔ1öhAAGN3FGL J0316.1-2611@ku‹y¢ƒÀLá@&`½À9™šMÀÀ;Ší~óûæ?¿^&"¸@'k£<"?ýµu_Óz;¿æ4©: >¿ÔS"™Tq¿¿ÓLw¿vš^¿æüv.õ$ÉAGNbll@¤zN¤¨ÁUPowerLawRBS 0405?ïþýöݹÑ? À5/A"?  –L¶°i? À5/A"?ïÕLlâxÓ?Œnˆ	S"Å?uYɁµ™?Œnˆ	S"Å?ïçm÷Ì¢'?b¸}×f™À?h'ù¤iR?b¸}×f™À?ïäÆÅvÜ?T=Ӈhtø?k9€$‹¤0?T=Ӈhtø?ïüTÄtÛì?<AÔ6$¶?=YÛí`:?<AÔ6$¶?ï"Kim¶?³Á3&ù ?›¶'Þ{L?³Á3&ù ?ïÊyʶ?€Mª¾")µ?zà+
p?€Mª¾")µ?ï^¢t€ý¹?ƒqÞ%¤ÿ"?"+±n(zé?ƒqÞ%¤ÿ"AGN3FGL J0316.2-6436@q˜Œ€AÀG` SÇþÀ9™m~ˆœÀ;Ƨ‰Fe?¿àáÕ#[W@)f],+@»ˆß¸ö¿æ¼ö‹ÝÕ¿äèåËæ¿Ømÿ!ˆ»Ñ¿Þ÷YñÁsAGNbll@›eø7´¢PowerLawSUMSS J031614-643732?ïÿ¬"—?Þk=8ÎW?
hÙô*Ç?Þk=8ÎW?ïØק=¾t?ŠÓ‡O_ѱ?s",a Æ
?ŠÓ‡O_ѱ?ïê>•<Ô?lÈ8²³ÏÛ?eÁj¶/¼?lÈ8²³ÏÛ?ïþWO?è]{Î?.¾!Q—A/?è]{Î?ïþþĨ³?ƒT÷H? bo(A?ƒT÷H?ïV¾ò³U?§ÿÖђÂ+?•(!²,bŠ?§ÿÖђÂ+?ï帔d.0?q?£—;öÇ?jGk"ò——?q?£—;öÇ?ï툥f½Š?Vo•õ'F?bwZ‹"?Vo•õ'FAGN3FGL J0316.6+4119@bÅ}q?À+xÃß¾AÀ9š÷È3áÀ;1‡ëlm¿þ?0Õ4û4@
Acôq+'?þlËð¦¿æb;qE< ?ïéå}Ya¿âÂÝÌ4² ¿äTæ–nä1AGNrdg@¹·KƧðPowerLawIC 310?ïú6|`E2?UPpþ_Æ?G&C.'v?UPpþ_Æ?ïÉcc|§?Š¯óò,b?{NNQz¦¤?Š¯óò,b?ï±	1yl?€ë›®—Žš?ƒ½³¡M??€ë›®—Žš?ïÿΏÎa>óÜAZ¯Ë>ø·þ`¬!>óÜAZ¯Ë?ïêl*¹.?lMpV˜S?e"ÕÚÇr)?lMpV˜S?îïÓ¸ï·?°{ö2«¾?¡Äw‹?°{ö2«¾?ï7¢bQ??""/݈?™kº•?""/݈?ïúy`i!W?Mƒ˜Ñ÷œÃ?F~qx$î?Mƒ˜Ñ÷œÃAGN3FGL J0318.7+2134@dZ{ 1ίÀ=¦B 6mÀ9CYLVÀ;FüÎX%¿ò%¶Ëƒ¡‹@ZaðàÓ??ýeŒ¿@)¿È†ÙI»h¿âÒÔ
³È¿ÚêYùN=®¿Å­åMn•+AGNbcu@¯"3¶E¡ËPowerLawMG3 J031849+2135?ïÿ¶62l?<ÁtSŸ?ryC[ìs?<ÁtSŸ?ïÒyELvŒ?ˆ>™WzF_?vÃ]8Èyþ?ˆ>™WzF_?ïæì,R]4?iáOž÷?iӁ§Ìl?iáOž÷?ïÿûÅPa>·lE%Â>ÀñÄ`h2>·lE%Â?ïÿ¬úZµ¿?¬Ò»p·ê?ÁcŽ")±?¬Ò»p·ê?ïb¿sóÃ?¢õõŸ7?"¼¨ɹ¬?¢õõŸ7?ïæAž8˜U?ud¡À†¤¿?i¾a­J¢¥?ud¡À†¤¿?ïÿãŸå>ìG
W)?_>ìaL]*>ìG
W)?_AGN3FGL J0319.8+4130@bґ"DžÀ*ƒ þ}IÀ6VdöúÀÀ:C,x.?úw°:ÅÏ@»ªõâoÌ?ÿŠ\º³¿Þza+OJ¿â%^>#Ò¿áXïYXz¯¿äĶ köAGNRDG@TœygËLogParabolaNGC 1275?ïãI½þ?|Q{Ɠƒp?lp¶5+'ñ?|Q{Ɠƒp?ï°]g¢?'Ø,
ü±?ƒè»¡??'Ø,
ü±?í`EáqÜ?©¬ÝþJ¯?´ÿõІ}¤?©¬ÝþJ¯?ïæŒ-—µ5?T|?uœža?isÒ'²#?T|?uœža?ïBÕ:"F?¡9h³F»?—¥XªìT?¡9h³F»?î›Æ­Nk?³°4ëEÿ?¦C•'°MY?³°4ëEÿ?í˜`Êx½4?¦§Ã«uk?³<ù¬¨	â?¦§Ã«uk?ïà	æÜB?fŒpü?oöÞµÄ?fŒpüAGN3FGL J0319.8+1847@d¢ß?–À?¬",2À9a6€Å=À;+£»[‹A¿ëq†œ€˜†@W¨ï¢æ?ù&:è¸?î¿^·ñH'?ÐG¢Ó¡t§¿Ñã%•L:¿È›ÀCì-AGNbll@¹èÍVPowerLawRBS 0413?ïÿe/Û?6gD_??¶¯t[?6gD_?ïÒÚa¤¤~?"JÉGŸ5?v'ÏHz´¦?"JÉGŸ5?ïÏ·¨£LÌ?~âŸT!Ø?x$+É&Ž?~âŸT!Ø?ïÿèH†à>Ü=¨Ë™p>ç·4ßd·J>Ü=¨Ë™p?ïÿm+…"?
Hü
ë?Z'Óƒ°Ñ?
Hü
ë?ï6sÑÖCe?°ù6B?™1…¾X[Z?°ù6B?ïÕÑøI—?'\@KÙ`?uø/?'\@KÙ`?ïÿŸÈûº?	HóÇ¶l?8ÀÔÿ—?	HóÇ¶lAGN3FGL J0322.0+2335@dCsÿ¬*À;—ý_;ϺÀ9P»Ú6BÀ;F>{?æ°5­Úñ@$Š
ÛPH?ÿ"«€÷·1¿àtŽì'Â"¿àUšéоŸ¿ßçÃô*¿× cڒUAGNbll@¦,:^5?}PowerLawMG3 J032201+2336?ïüâ;w-?2¨9À¤%?8î%®3ç?2¨9À¤%?ï¾ù=Õ3à?•"שÕ0?€A°2h	?•"שÕ0?ïØû6l£—?q{¥š³9ô?s'dÂÎüe?q{¥š³9ô?ïö¨ø9ì?<NÎdüt?SÞ­†ɛ?<NÎdüt?ïöêÎ%Ï?Q`1F0ªZ?SÊ*Ì('k?Q`1F0ªZ?ï2¯>5^ ?°_Åé¿Ýâ?™ªAë1è?°_Åé¿Ýâ?˜ðQa?Š¸l#±ä?‰•YÊÊߥ?Š¸l#±ä?ï®D*T<?tòޞÏ@?"nû0C†ì?tòޞÏ@AGN3FGL J0323.6-0109@fþßÞøH|ÀFœäÿÉy[À9tJLTliÀ;i'Q¦»Á¿Á7ð㓞ê@
¼¤ªnÓó?ý¡¾ Œ'u¿äv%7êI'¿Ú'e»4Ž¿ÑíÖ/ª›'¿ÐñèŠÃgôAGNbll@§ë0¾
í)PowerLaw1RXS J032342.6-011131?ïü¦Ègs"?4ünHtÇ?:ɺ·ëØÍ?4ünHtÇ?ïÕBíes¢?‹2œ°0|"?u^‰DW2ð?‹2œ°0|"?ï̓JÕ^?sa"V!x?y>~ëÃ]?sa"V!x?ïùÅÂ}¤­?3ñF%ø?Hè÷ܤ?3ñF%ø?ïø"¤"{?I+ýKa»3?M±n+?I+ýKa»3?ïur·œS?³òßkÙï?œ1Q¥œÙ«?³òßkÙï?ï¬?cºz?ƒöýª¿¡‹?"ð'5r)r?ƒöýª¿¡‹?ïÓrE—¹Æ?gÄYŸý5ž?vFÝ=/?gÄYŸý5žAGN3FGL J0325.2+3410@czªŸ{ZêÀ2±Þ_œGÊÀ8ª_!ΆáÀ;r‰EŽŠ?öÖÒµ'@º³PÏÑ9@¤Íˆ´o¿åÖ2¼•Çþ¿ëÕf7I¿ëp§
ׅŸ¿å)y<¤AGNnlsy1@nr†/YŠLogParabola1H 0323+342?ïþç{œ%?%Í	Š"â?!ˆE>™d¾?%Í	Š"â?•É?TD]¤ŒA?‹V¸ÝýWÌ?TD]¤ŒA?î(xU?'öböVøL?‰XDk"¶?'öböVøL?ï) f8)x?wµãÐj(L?šÛó>":î?wµãÐj(L?ïúÔ­Ÿh™?FM¢# ?D­J€ZS¨?FM¢# ?í*°à)˜L?»ü¸'›7B?¶ªxÿ$?»ü¸'›7B?ïZ;»Ê?'ÙƒQt5?"¸ˆ"†Ø?'ÙƒQt5?ìaŽ_v)Ÿ?©úLK'ìK?¼óN³?©úLK'ìKAGN3FGL J0325.2-5634@pí ßÞøHÀHîà_PÈÀ9ø¦wÎm·À;øñ¼p^7¿ó¼lzQªÃ@í«B¹c@¹´ß›0ž¿ãu'ªMW2¿ÝÊÉTÊÚ¿åxþ(º^`¿àX ŽAGNbll@"[
Ú¹õZPowerLaw1RXS J032521.8-563543?ïüv[""¬?:ß!uØ)Þ?<M%]PZu?:ß!uØ)Þ?ïÕwj3"F?*ZÚ\¦v?uDJíÅ?*ZÚ\¦v?ﳟ…•ö?x:î:s*?ƒ¬«Ö›?x:î:s*?ïþûÐë¯?ß}ºŽuŒ? N"@«¨?ß}ºŽuŒ?ïö³"Á	9?SÈΰ½¥¥?R˜öô a?SÈΰ½¥¥?ïT¢wA]¡?ª³RÈ6Ö?•k±CçÜ?ª³RÈ6Ö?ï'õG?Y²?"iLØr]Æ?›W5'Å?"iLØr]Æ?ïâT¤O³¥?h›(óé?m«[©m"ø?h›(óéAGN3FGL J0325.5+2223@dub¯È°À<I¥ÒÀ8hpeÓÀ;Rs×Ûõ?õWéÞ«qˆ@BFBÚp#@¡êöÙe·¿ä¯ñuVKð¿é1-o#ú0¿èæ¨ãZû¿ïÿ?"éøñAGNfsrq@sÎp:ûLogParabolaTXS 0322+222?ïúô§?DjœD†z(?G¯ËÓÅÏf?DjœD†z(?ï¹6@j£?…ÕàGý½?²oÚՍ^?…ÕàGý½?ïÒrG?Œf6¹Ò("?œ¥¼AÙ!?Œf6¹Ò("?ïNäXsxa?uó‡‡'p?–#tøp+Ç?uó‡‡'p?ïö¤ô¸ñp?Spö2Ü×?R¶ãSof?Spö2Ü×?îpª¶nß?¸¾r&õ?¨ÿ•RáD?¸¾r&õ?îó…´Æë?—Ñ,8ç? Ç¤²»úN?—Ñ,8ç?í¶Œ´Xâš?ž'I¸jF?²Kš\]/?ž'I¸jFAGN3FGL J0325.6-1648@iÀÊ`ÀJy¢@1HwÀ8þ­-]À;.InÞÚì¿Ý4gX\@ØOØŽZ?üì¿[u?¼â¯ã ܿޙ`æÂ
οÚìýf?¿É÷7ô&óAGNbll@¨¶XüPHPowerLawRBS 0421?ïþC"cÛ®?$¼¡ºÄ?+ÆËÒ	 ]?$¼¡ºÄ?ï˒ób7Ù?¶0áÆÅQ?z6†PCë¹?¶0áÆÅQ?ï䫧IkÀ?ešQ".:7?kTXÍñ—â?ešQ".:7?ïÿSÐ6¹¥?Ú®UùÉO?…õÊÆî'?Ú®UùÉO?ïþmbrÕ¤?#Ð)ïM?))Ø"¹»ê?#Ð)ïM?ï `@î™?µrØõnx?›îy2Ø?µrØõnx?ïà¢5Z»ô?y7¨i¿W?o]Êoª#×?y7¨i¿W?ïûåƐ??6‡+ÀCu?@hä̒Gh?6‡+ÀCuAGN3FGL J0326.0-1842@iý^ß)ÀJÉ?Àà0À:P3:~À;ê'Ô©:!?̐õ_ß'@"KtG¥†@¤ìԍ¿ç­üÉÙl1¿ë¨ËÓJß?Îq€Ö()¿å)Rü{;AGNbcu@ŸƒÚkP°òPowerLawPMN J0325-1843?ïÿ£•µ£)?ØܛI§?‹%ùÔ?ØܛI§?ïÓÉÙ?‹‰†].?vs›.Je\?‹‰†].?ïæómå$¡?pÇJ»'Î0?i'%Ú¸?pÇJ»'Î0?ïï¤;šF#?LpW­ž?`[ÄLü­?LpW­ž?ïÿ«Ë#ä>þ¢m®þ?
%oæ(ú>þ¢m®þ?ï-šyWH«?³'ŽiÑ3?šL°Ï?³'ŽiÑ3?ïÜEy˜§?t'Âu[ýÒ?qÝCN´l?t'Âu[ýÒ?ïÉÑ…6?x¬U:òØ?{u·ò%?x¬U:òØAGN3FGL J0326.2+0225@f—ðŸ¥LUÀE7´_î}!À9^9£¼¡À;sK@p2˜¿Â2õö¼µ@Pß:šˆ?ÿøaՈ]¿å>êUÁ¿ß‹ß¼éá¿Ù¨ÀdDß¿áà¼:OÔAGNbll@¡Á¸Që…PowerLaw1H 0323+022?ïþÂä3=?ôI"õ?#ØÞí+?ôI"õ?ïÉ
·'Òr?'‡ë'c?{z¤=6ï7?'‡ë'c?ïép¹rõ7?auk9Ns2?fF¥Çøl?auk9Ns2?ïùC"'º"?2ǔƒˆ±_?Jñ²j>ͤ?2ǔƒˆ±_?ïýc·Å?2M?Œ§?4âH\›÷?2M?Œ§?ï,HZ.A(?±Fzdnf?švô¸€ö?±Fzdnf?ï֙
úáÕ?yÿû®M¹ÿ?t³xöài[?yÿû®M¹ÿ?ïχü}y?eúù…Fq?x<Ökk?eúù…FqAGN3FGL J0331.3-6155@qO{`(^ÄÀG)´Ÿ¯]PÀ9¢ó_2•À;Ãþ+êi–?ßʆ˜ØJý@JêßÝK@œÁ€hp,¿Ûh€{¿áýý–æü¿ÙS	÷>0¿çè0ˤٔAGNbcu@›ýɅðoPowerLawPMN J0331-6155?ïý_ÿ;X?6QhhwJS?5sÙÊ?6QhhwJS?ïÎl†ÞMu?ƒp\†¸v?xɼoÝž?ƒp\†¸v?ïè=t2_?f³J>ðZ5?gŒYîb?f³J>ðZ5?ï—|Fޜê?f^˜ Ð?Š îR§™l?f^˜ Ð?ï÷C]Í»Š?Ucá::ä?QyDÝ{*ú?Ucá::ä?î×ZD¼j?­öB³v?¢Ú_#Õ\?­öB³v?ï'ëÁÉR^?ŒZæì¸Äe?‹…ƒ\"¡?ŒZæì¸Äe?íšý›2I?—D/¤'?³($·ÿ½?—D/¤'AGN3FGL J0332.0+6308@a~] Y§;@Ø4¤À9Aq
.W+À;E}ö¥ä+?ډWw`3Ç@
~ºÆ@¥àŸgŽÚ¿ä@Ë·€¿âbƒp'o¿çü5ïêÍØ¿áx¸É	É­AGNbcu@"ß!-w2PowerLawGB6 J0331+6307?ïùI¾¡!4?Uv¥Ê閇?JÙ°Ÿœ?Uv¥Ê閇?ï¼ÓFRd?‰úF'ªÑ?€üK!\ã-?‰úF'ªÑ?ïƒ	«^?w\¹ÃËfY?~¾{Kˆé?w\¹ÃËfY?ïÖa@aÄì?W2%TÂáÒ?tÏ_å	à?W2%TÂáÒ?ïÑZë®?yª*	£9?wR¹%Eá?yª*	£9?îqòĒZ?±uö'¹êX?¨àÞáÿ[?±uö'¹êX?&:ô•?ÍÍ-
âé?¦Užäk¬?ÍÍ-
âé?îwñÙv©U?"JÄŽ¼?¨€âjM8³?"JÄŽ¼AGN3FGL J0333.4+7853@`Pz WŽ\@2{Ä¿¸TÀ9Ç~è=k›À;Ìëô°@¥¿à— ïèõf@%Ê>ýí@"Äÿ£ä¡¿Û•Dí'6›¿èñ%Ž¿Ôº˜ñí²d¿â_†«ßAGNbcu@˜'¶z—PowerLawNVSS J033344+785027?ïÿLbƒV?ƦN¾ä?s¼Oóg5?ƦN¾ä?ïÙn0è³¼?_¾±H
h?sH燆š*?_¾±H
h?ïë4ë³Ü€?ckÄ{%€?dË (€†?ckÄ{%€?ïüK—¥p	?)´õæÁ8(?=£DÏ_¯;?)´õæÁ8(?ïþ¢»^îÖ?4ãöß@Ôô?%ÔHm(k?4ãöß@Ôô?ï%çTQTË?°XÄÈ^†?›CreÊ ?°XÄÈ^†?ïßX‡¢îy?t9	'oBÊ?pS¼+ÉP?t9	'oBÊ?ïÙå‡ó?i,kó3þ?s
zOóüp?i,kó3þAGN3FGL J0333.4+4003@c3›Ÿ˜·À)óš?±Æ·À:ã'ñ·À;"b£cF÷?î…pƒ[û»@q¡Šÿ¢ã@æ¿ßÿY'?ïý°´,0Ï¿Ç$ۛ`‡ï¿çþÏ$¯¦¿ïÿ	ø&mAGNbcu@œ1ôêJŒPowerLawB3 0330+399?à†Re¹©k?ÎDI³È:?Þó[4Œ­+?ÎDI³È:?äŽs¸ßZ?ˑÅF½öè?ÖãŽAKÐ?ˑÅF½öè?ç6—$
??²AUâ×ói?ѓÈÑ·å?²AUâ×ói?æ%Xç?¨W×C¨‰<?ÓÕ´áãN2?¨W×C¨‰<?ÐÇ5âB³a?ÉzK—ûVD?çœeÞ¦O?ÉzK—ûVD?Ôó{¸26?Ï£v'-•?åò†B#æå?Ï£v'-•?ÝÝÉâë$Ú?½ÚL$×â?áŠm"?½ÚL$×â?ÌJz"€6,?®érDÍ?èía[òu?®érDÍMIXED3FGL J0333.6+2916@dªKÀ5…šr¦çÀ8ÉðeXImÀ;=¨;i?ï-@ÓÃ6 #?ý¶É™"{¿ÏgÆ°_¿Ú¦¸f
{¿ÕNÇ,ò|¿Ú‹Ù"׬‹AGNbll@§a"MÒñªPowerLawTXS 0330+291?ïÑ{ýɼD?ÞÝOQ?wBSªQ?ÞÝOQ?Œá?9ÌÌÄ5Ç?‰úÞ§!?9ÌÌÄ5Ç?$~}?"K."7ml?‹'vÏ.Õ?"K."7ml?îéy8¿Ô?uºöÿ¯ÜÕ?¡nøifÇ?uºöÿ¯ÜÕ?ï—ÅØ֊*?…º
Kċ?Š‰À¡¤?…º
Kċ?ìüƒJfšX?¸¬cåqx,?¸å­§B?¸¬cåqx,?ïÊOç@c?"':ÿ
?œFµýð‰ª?"':ÿ
?ë¶zÙm¢£? 5s2ç?Á&šIur? 5s2çAGN3FGL J0333.9+6538@aUDupÅ@p4 ½À9SFS¡hÀ;YÜ&Ü㛿ë…hßÜ@•ÒóW{?ÿ-! a¿ágZ™t
¿ã;©MZ•'¿ãEMVlj¯¿Ã3{}¸AGNbll@±=Ø˒:PowerLawTXS 0329+654?ïüÒ@ª;?4)¨–`:R?9múÖó@_?4)¨–`:R?ïÇËÖ$0Ù?ŽI£¥³?|áˆûx?ŽI£¥³?ïÒ¦´×…?sÀ'ž4?vü,º1åa?sÀ'ž4?ïÿýï¸?pin¯?@ÌTù@?pin¯?ïô¸æÑ?Sy¤d®j^?Vðm@?Sy¤d®j^?îãöÁV»½?±Î^FÖ·?¡À"ê"D+?±Î^FÖ·?ïjS€…¡j?þ À?'µí"¿?þ À?ïõŒ"|pƒ?Sàw»­‹?Tçºö Ú¥?Sàw»­‹AGN3FGL J0334.2+3915@cG_ét£À+Æ 
aƒÀ:3æ/tbÀ; Öwpyæ¿ñ[µ
8h&@	'C¼˜L=@èØÞ\—¿ëž"('D¿áî‰~ª'¿Ñ§ˆUà˜¿â®+VÅßsAGNrdg@§jÍÅÖ8†PowerLaw4C +39.12?ïþÚ҅.º? ²¤þ¾w?"RØDÏðz? ²¤þ¾w?ïÁîJS"?'üÒ[Ô}u?õ£)î?'üÒ[Ô}u?ïÔ®Ý<uk?x
YÅ[¦?u¨'lÄ
q?x
YÅ[¦?ïý™¢Cv?$:vñ)åþ?32ï¯ú
…?$:vñ)åþ?ïýs²™¿?1.À|ÂP?4biŲ?1.À|ÂP?îˆmˆÒ?µ÷0¯$9?§y't"CÍ?µ÷0¯$9?ïÍ~æ»?z&m!–?y|qÁ<Ž?z&m!–?ïÓ4'ÆÖ-?sd@ÈýGY?ve·8ɔ?sd@ÈýGYAGN3FGL J0334.3-4008@n˜ºà;>šÀK{Ÿ³À7ã$Õ¢^dÀ;ÁÀ)P[?÷	ÿºùf@
PIC•×@΁,æ=¿Ü¤SÃႿãoç‰ðõ¿ãT!šsx¿ä2Ó:éϬAGNbll@¸QC¿rqLogParabolaPKS 0332-403?ïþjÂ}?TR͙±°?/>õ•!?TR͙±°?ïÑ=­4¬?Š2*F:üõ?wa)hi­ç?Š2*F:üõ?ï¢Ò)ñè?ˆž?0üo?‡KuÆÁõø?ˆž?0üo?ïê
ÜÝ?MJ÷Såü³?eò#î!©D?MJ÷Såü³?ïþ$БIá?,Ì-ñ)Ö?-²újbm?,Ì-ñ)Ö?ï$ª*Ñ?²• 4I{?›jº¾?[Ú?²• 4I{?ï'+zC?÷9]'?‹u=!|/.?÷9]'?ï×»\{Ÿ?g«µr¹?t"QãÉO×?g«µr¹AGN3FGL J0334.3-3726@n¶â—ÀK.Æ 
aƒÀ83A!…À;é/"Ê?òd>0<]Ô@@WŸÏÍ?ÿD@v½¢¿Ù?…¨Ö'¿ÞÐY©êt¨¿à
ƒsVS¿áÍróéAGNbll@–Û`uöý"PowerLawPMN J0334-3725?ïÿ['‰B?gàim£?ÙÝ5õ?gàim£?ïäïÛg?Œ}$Ɲ"?~-‡ôçÁ?Œ}$Ɲ"?ïÈŠ1r?{#Š¸6?{ôø¼G ?{#Š¸6?ïiϤÃnT?pê¬Aùõ?'Æd"™|?pê¬Aùõ?ïÿɑȯ?µ–Keå?ÑtÀ¥?µ–Keå?îðP.¸òr?±,§ˆ,¥? úý(¦á?±,§ˆ,¥?ï.z¢ï•?"Ùáö94?Œ´aSÔ~Í?"Ùáö94?î	•^»;?•µŸíBN‰?¯fª¸™w?•µŸíBN‰AGN3FGL J0335.3-4459@o–``þG™ÀJs^ŸÈ‡ÄÀ9Èi*–¬À;ŸÈå·^¿ÿ€˜N?þô@ÅC–'¹?ýL ?µ?DkYÀ;¿ä3JJZ¿Û¹69y¿ÁíõçMWAGNbll@¦niᰉ PowerLaw1RXS J033514.5-445929?ïÿ9>/H?÷SÐS¤p?ØDÐر{?÷SÐS¤p?ïÓÍA'Æ?‹®¨ÑCIÄ?vu™t"±?‹®¨ÑCIÄ?ï× [G×ä?x
Á¼|ãJ?toÒ]sæ9?x
Á¼|ãJ?ïÿþtÜî%>§[T£>¨µ}ÎXæ>§[T£?ïÿcŸ%Žt?±ìħNu?ŒP
Å*?±ìħNu?ïO‡hÙL&?±ŠÎÃ¥O?–ëµ³:?±ŠÎÃ¥O?ïÌÎrÇÑC?~xú©7ü?y˜ÆŒù'?~xú©7ü?ïÿêö¥Û">ì+5
Kv>å	M­3U¡>ì+5
KvAGN3FGL J0336.5+3210@cã@¢‡À2ß?@‡¯ŒÀ8¥ÎÆ¢aÀ;£êUt?ð"éŒùM@†GqD@ÿ•!¿éÅÉjý
¿é—£‰â¿ï50ZÞj¿ïöZNÍdðAGNfsrq@s&t}€^_PowerLawNRAO 140?ïú¤{ÊÑ ?FbÂm,@ì?EnY"M·?FbÂm,@ì?ïXTÅuÉ?–8üÔZy?"õ|áªã?–8üÔZy?îØyc÷©Î?"Ñ̊ŒS?¢xià ?"Ñ̊ŒS?íܪ†·ûÁ?Š·NŽ*?±«È`~?Š·NŽ*?ïõͪ Û‹?Z_P¦ÃD)?TdªßE*?Z_P¦ÃD)?êÿÊ 1ø?‹m[øú'?ÄÕ›8"?‹m[øú'?îQ'>|? èFÃm?ªîwÚfš<? èFÃm?ã1LºT
?µŒ{'Â??Øåf‹Wë?µŒ{'Â?AGN3FGL J0336.9-3622@mÉõÀv}5ÀJó²ŸúÜ«À:XSy#ØLÀ;ç@Çplz?ãoú¯@Á@«"ªO@}¾€ƒÈø¿ã¡EßL$¿äM՝Î)¿í2išV
¬¿ïÿ¬vÒ*–AGNfsrq@‹
-à
PowerLawPKS 0335-364?ï¼}æ¤~?‰×<îÁ?€à†a‡E5?‰×<îÁ?í+Áþxҋ?¶[°&;?¶¡ð
«?¶[°&;?îÐãTE?—™røÞ9?®îBñÊ»®?—™røÞ9?èoê^-1ç?§GŠÒ?Î@V‡K8c?§GŠÒ?ï3ɨ·^?¤®v¿\ÉE?™†ÜÉ1FP?¤®v¿\ÉE?ڎu…ÝÐ?ӇÔ=Ú?â¸Ås½?ӇÔ=Ú?ìDѬÁ¥¸?¨Nœ8bû€?½Ùr™òÒ<?¨Nœ8bû€?Àjg…}á`?©Œ!€Á!?ëåf ‡¨?©Œ!€Á!MIXED3FGL J0336.9-1304@i+eà.©aÀHr¶?¯À9÷×fƒÂ˜À;Ͳ¿-?¾ÔT1Qÿ@
I—è¥#@\ 2e¿çœX¸uIP¿è
LTþp¿ì,í4‡'Q¿Û Kb\ŸAGNfsrq@}_á\¦ÊPowerLawPKS 0334-131?ïý""Ôb»?QÀ,N<L?3fël®'¾?QÀ,N<L?ïȕì¢r?'˜Æ•8&†?{µ	¹F›?'˜Æ•8&†?ï—Tè|?€½¿¯&"?Š*ûÓ¶Ñ?€½¿¯&"?ïǗ¾Vè?eìðšc™Z?|4qGè?eìðšc™Z?ïïD3‹ž?fî ð¤ã?`â»ÂÕz`?fî ð¤ã?îÁ‰€Oy?µ¯= Rf?§ãçegSo?µ¯= Rf?î´I/Žì?™éRï…Q?¤»nOšÆ5?™éRï…Q?ëÑ×w	?²¼¥€`@:?À¸¢#ç÷Ý?²¼¥€`@:AGN3FGL J0338.1-2443@k\_x5œÀJNVßà¥ÈÀ:Ç×-xßÀ;Çå–È.?qê™*üµ@µ
a½_G?ô"=!±í?çÚ«»ÁGð?îàÃdCK"?Þ²~àä9"¿¼y¤Ëj¼AGNbll@ÓíE¡ÊÁPowerLaw1RXS J033810.1-244337?ïý'ÿ´'Ô?D!­aä£?6ÀϞd`?D!­aä£?ïÛÛThÑ¿?'Ðûšêv\?rUÈ'"P?'Ðûšêv\?îŒØPÂñ?¡Sé4?§2zör5ó?¡Sé4?ïü™¦"¹Ž?)¤n¹Üá?;2Íõ×W?)¤n¹Üá?ïý4ž1?FYQÑõۋ?76].¹6Ò?FYQÑõۋ?ï/'eI°Î?³ûi×ÚÓé?šX´;?³ûi×ÚÓé?ïWµrìn?" þpfx
?•	Q¸YxA?" þpfx
?ïûv6¤=?=ËùJ?B'%J6#Q?=ËùJAGN3FGL J0338.5+1303@e±ú€Ïž8À@uç_ö	ÝÀ9R&"©x4À;+_ùdÛL?ãyc)?@M<yØÞÿ?û'Àä6K?ÿ
¿ÀpÎ^È7g¿×ë´Š¥z¿Ü
{ÐA1µAGNbcu@¶Öèõ\PowerLawRX J0338.4+1302?ïýŸõB%®?*aÞ,PŠ?3T²)á?*aÞ,PŠ?ïÏIÇIU4?…ÉÚ?><?x[urn?…ÉÚ?><?ïÑ-[F¼l?t÷ x1Ê?wiREDr>?t÷ x1Ê?ïÇáøÐX??^œ"ëR‹?|S@z?^œ"ëR‹?ïúSÑ
y:?G—!V¡vz?F°¼U¾i#?G—!V¡vz?ï9o˜g?ª
ä›ÕÇ?˜Ònªël?ª
ä›ÕÇ?ï¨eÄw`+?†Â¶T°ô?…æŽâ'õ4?†Â¶T°ô?ï@b%Ë'?Öµêï2ä?—ÿS¶1*?Öµêï2äAGN3FGL J0339.2-1738@j\¿ôw6ÀI"l?Ä;.À9µè«î0À;Âóá?âEz°AÉ@§¤d"ê;?þÙeÿä&[¿³ó€çWMÖ¿åù25Ý1Ÿ¿ÑÞh_S¼Y¿áɱD00ŸAGNbcu@¥	¦€IRPowerLawPKS 0336-177?ïþØ]Nº£? €Ä?f"Ç?"z(Ñýöð? €Ä?f"Ç?ïÐܶú¨}?†HP1fm?w'¤<%i?†HP1fm?ïäß±3œÃ?jI'^Q›?k Nµäþ?jI'^Q›?ï¼e'ÝÁ?\ô©99§€?€æ›}9´?\ô©99§€?ïýè‰Irî?-d¦kÉ?0»µÔKTT?-d¦kÉ?ï.øáӚ?¥D8~Ón?š>`èìöµ?¥D8~Ón?ïÆÒ$$¢w?€–ÏÞ!Ð_?|–îZðu?€–ÏÞ!Ð_?îÒà{fŽæ?‰À©ÓÎsÁ?¢ÑøM┓?‰À©ÓÎsÁAGN3FGL J0339.5-0146@g€À
¡©ÀE9…¿ÈŒÀ7êûgPÀ;Ao¸õs?ø
ÃÁ
w@1sHL@«,Tò œ¿âBü÷Àt¿æ=ä²F¹£¿æË°ŒÇ›'¿îB"¼díAGNfsrq@uµ^ñýßLogParabolaPKS 0336-01?ïÞÍey?j2 §ƒ?p™MF?a?j2 §ƒ?ïÎ98Û¾­?Œà¾RRáŽ?xãc†qý~?Œà¾RRáŽ?îÑ2sV?˜r–@5ߒ?¦."ë ü£?˜r–@5ߒ?ïë¾`9@?O?Ô$?dAï·$_?O?Ô$?ïÊ<—5X?xHZ¢cóÀ?zᴆtÉ?xHZ¢cóÀ?ï$í[sÕ?³Ç)¯,Ò?œ{b[p½M?³Ç)¯,Ò?î»áLX¶?˜µvâ
ƒ?¤Aë8Ææœ?˜µvâ
ƒ?ïß¿4Öò?eâ³î¡_>?p exÇ;d?eâ³î¡_>AGN3FGL J0340.3+4130@c9 _ñØÀ&;¹ÿkÀ8‡"õÎNÀ;YnÉw-@shÁ_†@qÁ:Gz?úAÔ£ÿÏ¿Ð$ð¿ßî¿Ïéx¬0—o¿â"‰ü²\x¿ê;õ2,ßPSRPSR@•CbMÒñªPLExpCutoffPSR J0340+4130?"`œ?™ßТ©¿€?ïgå1‹?™ßТ©¿€?°&·'?ÂãùnìFæ?íû)Í¿€?ÂãùnìFæ?ÐM‰¸G|
?³oɜ®±`?çÙ;#ÜAú?³oɜ®±`?±RȵG?'
3sg.?íÕ¦é@ÿW?'
3sg.?‹¦iX*°Ð?Št
+£K?ï'fZä
l?Št
+£K?"mFÐ*­?ªÆG'.Îò?ïd•ÉUsû?ªÆG'.Îò?±Z{Î6í?­ùcè3â?íßt°½2â?­ùcè3â?‰˜[·þâÞ?wa¹4æK?é
µ?wa¹4æKPSR3FGL J0340.5-2119@j¹ fèlÀI—Ï¿ÆT
À9¨¹t*tHÀ;ƺ_ÿ¿Ó"(h@!͌Fµ@½j?¹ÔM¿æîNm)Þ¿Ø22ä{7¿ç§›ãõi¿çuê	k)AGNbll@"R§ï²-PowerLawPKS 0338-214?ïýe-M¸g?;Km¥aÔu?4֓oÇ·?;Km¥aÔu?ïÛ³zì/?†Èj0ƒ'(?rt&-ì@h?†Èj0ƒ'(?ïµí3Žf¤?€¦T=Èü?'"³wZò?€¦T=Èü?ïǿŴÍ?6¿ºœåÓ?LÍù:‰ò)?6¿ºœåÓ?ï÷o""O‹?T复ҵ?Q Øçß	'?T复ҵ?ï
֑`~à?µÄÉ=ä ­?žE-ÙŽ?µÄÉ=ä ­?ïW7âU±?'-'XT!?•9
"Í?'-'XT!?ï¡JˆJ£?xê2¿j¢?‡¾-]íWB?xê2¿j¢AGN3FGL J0342.2+3857@cu¨ÙºÀ)¡ÃA2Ð7À9c2:å¯À;sƒY¼3ø¿í$GÎÜؚ@8rP)Ž@ôR?gôÜ¿äSõCŸ£/¿é%©K­¿ß6Á¡å1¿á	pe)
ÌAGNfsrq@'mlô!PowerLawGB6 J0342+3858?ïÿÛ÷@>ð#¢ðm¼r>ò|–:†š>ð#¢ðm¼r?ïÀX±X8b?#֘Ao?Ó§27£n?#֘Ao?ïð^ÈôaM?Xv‰ÅÖ)?_Bn-:æÓ?Xv‰ÅÖ)?ïÿï,%Ö\>Ññ·0á>àÓÔß¿°>Ññ·0á?ïÿÅ$.Tô>þS0®ˆ´%>ýnP£Ev>þS0®ˆ´%?îðh4O?±éŒ'ïqã? þÉz+?±éŒ'ïqã?ïå¼~1D'?o¦3ÀR¿5?jCÝÙÆ ?o¦3ÀR¿5?ïÿŠ•"o?ؽCÖÓÌ?
Zº®ª`?ؽCÖÓÌAGN3FGL J0342.6-3006@l|¡A(¿ÀJCr_˜ìËÀ:Ûk3TÁ"À<?'æFñ¿æmŸÐÀLa@ދÞðæ²?ý‡_úfŽ?ïÿd"$©>¿ç¡jé?¥d'qya¿ãÈï˲ùðAGNbcu@°lPÿ—$tPowerLawPKS 0340-302?ïÿT,ÉF?0®%ÔIÛ2?zy\í?0®%ÔIÛ2?ï×m˜É™?‰ªßjÓq?tI}›ïÕ?‰ªßjÓq?ïŽñÀª³%?ÕÂïÈ20?ŒCÎsþÆ?ÕÂïÈ20?ïþ§q¸Bì?Á‹k
º?%ˆâ^ے ?Á‹k
º?ïÿ™Þb÷F?Ô¹ù¥/Á?	ˆg*nœ±?Ô¹ù¥/Á?ï6ɬ˔W?³)|«®6b?™&Ê_®=?³)|«®6b?ï¢ûhWÇ?‡íÍ'àì?‡A=08â2?‡íÍ'àì?ïùçß;©?E™/Mã?H`ƒgӓ?E™/MãAGN3FGL J0343.2-2534@k"$?åÉÀIÓ½ÿªo«À9dïS	'À;Áozân?õIu"¼gÐ@ÝŽ<_@z®YÒY¿à«îz
vë¿æ™,¡É"Ý¿î\+~LÐØ¿ï夦Î;AGNfsrq@'R}ÔAPowerLawPKS 0341-256?ïö~øêž*?SΣuÀ=t?SV¾«\?SΣuÀ=t?ïЍ,Šç?"Ôžíi‹?w¹i­íˆ_?"Ôžíi‹?î² ºh–?"|™Jí£­?¤Ýô]ý¢?"|™Jí£­?ï­ii>÷¦?h2
lBÕ?"¥¥°Bj?h2
lBÕ?ïû搦?EPödæ&˜?Cœha®gÒ?EPödæ&˜?ïD+ËWN?­àŽ¨RX¸?œ÷z‹¼€1?­àŽ¨RX¸?îžR;"´5?œ»l¨í?¦ÜCE ²?œ»l¨í?î¿<)}?"ÝìïÃL?¤Œ>J.?"ÝìïÃLAGN3FGL J0343.3-6443@qsb¯È°ÀEԛ æÀ9fÖ 2¥oÀ;´UhaQ¿ÖYÛ¬AD¡@ÌÝÚçÐ@;}ßÔ¼Z¿Î² yL¿æh»j—¿Ül3,۳οåÿ3¶AGNbcu@"Š»²þÅmPowerLawPMN J0343-6442?ïÿÇÃE>ûÂ'QŠ2>ü^_èž>ûÂ'QŠ2?ïÛ'öê¼?ƒÿñõ µ?rl€°N?ƒÿñõ µ?ïêlÆ Ÿ?cú–Wo{'?e"âq¸ø¯?cú–Wo{'?ïýp«[/s? 2Z«‡"?4z£"ؤX? 2Z«‡"?ïÿÑ?‰i>ô'"‹B«>÷`*•Š…>ô'"‹B«?ït ÐÒbZ?¤ÿÚyÞ½?'{åãûæ¶?¤ÿÚyÞ½?ïêÉȶh?pòÁá³Ð?eù6v'gø?pòÁá³Ð?ïí®ÍIJ?S¢öÊU-ï?bQ2j:ýF?S¢öÊU-ïAGN3FGL J0343.3+3622@c°ƒÀ~à±À-fLÿyÀ9Õáƒ=6ÂÀ;x?ǖ,'ÀXî$`\Œ@ßE	¬§@i0`¿çWœ=Q³ì¿çޔiÂ7¿áÌøàÀ¹]¿ÝyHª­óAGNbcu@ŽrškP°òPowerLawOE 367?î?p}ìiö?Ȓ»õË.ù?¬ø¥«¢?Ȓ»õË.ù?ïÃ֘õÒ!?"+™TÝú]?~³$3S?"+™TÝú]?ï\±/H©"?"ßÛ׳ƒñ?"iÚêÛ´?"ßÛ׳ƒñ?ïÿò¤«N+>Ómoìà>Ú¶Ù_ðpE>Ómoìà?ïÓrb.?ŽjBR°³?v~À??ÄÞ?ŽjBR°³?ïš,;:?¦v2êÁ‡þ?œºq­ È?¦v2êÁ‡þ?î¯=<Bó½?ŸC˜¶8Äi?¥,:ö3?ŸC˜¶8Äi?ïþ*ÚÁy?."pó¹y©?-RUFOÎ?."pó¹y©AGN3FGL J0345.1-2353@kEi_ªŠƒÀIm|_Ìï1À9Bn
Ÿ–3À;ªªùš‹?æé»áJ»Ä@{Ú\S=@CU_'òc¿âýږ‡Ì¿æë)ʏí¿æ2ًn€¿åš\Y""BAGNbll@‰,ÍÒñ©üPowerLawNVSS J034518-235218?ïüš"GM¥?:lï›D›¼?;+d7¹²?:lï›D›¼?ï¾Øûb?'<|ç>	?€Iù¼ ¯†?'<|ç>	?ïÐb"'ª?sf³GQ?wζkhW"?sf³GQ?îÀ_¸ï—Ÿ?€ –úâ«?£únrÑ
?€ –úâ«?ïéXH7ô…?m k|p)?f§·ý¥bF?m k|p)?íM[T(e?·ØN|Ž¼?µ•%]	l?·ØN|Ž¼?îtG:&Aˆ?¡8ô~w³?¨»ŒZ,K?¡8ô~w³?æåd3íS'?¯gz7©†?Ò57˜%XÞ?¯gz7©†AGN3FGL J0348.6-2748@l1~þáÀIr¬¿ç<À:ëWÒNíÀ;ÒþÈÈ[N¿œ@2 îÊê@ƒg5™?@6Ÿú0Þ¿æxxi?¬
¿ã›åGO¿ã¹Ý³h¼q¿ïÿÛå:úAGNfsrq@ŽÓڟ¾vÉPowerLawPKS 0346-27?ïøsyt`$?MÎ2¨'?N2¼²ÆP?MÎ2¨'?ïÈ¡þîï?‹êš_Š?{¯~é+0'?‹êš_Š?ïê'óvÉ?à4`¤?Ÿb­Æ¸Ê?à4`¤?ïºBQf؅?g81ç-*?ok—Û'ã?g81ç-*?ï봇9M\?v¸lû!e(?dKx'x"?v¸lû!e(?îäÔ3¯–?±)Õ;ô1r?¡²¼ÃNМ?±)Õ;ô1r?íû^ñ?«¥ÅEö­'?·h%
˜©a?«¥ÅEö­'?ìÒ1;>øí?¥z-¡+'Ý?¹nv&v,?¥z-¡+'ÝAGN3FGL J0348.7-1606@iè¾ß¤?æÀGË <¶jÀ9wÅüÀ;Ä	Ñ:×?çt[5}2@ڗ.u0@»#à)¿àx7YáÀ¿ç'fÈHr¿è2ee4¿åH6¿H™'AGNbll@'v -à
PowerLawPKS 0346-163?ï©ðGüg?¹ÏO3
?…ƒîLÿV?¹ÏO3
?ïÃju¿Ÿ¾?†Óý1ˆR
?~JÅ"?å-?†Óý1ˆR
?'É?|tÀV¹?~¸»ï—Ž?|tÀV¹?ï$
¥Hé?ueÿgu?›~KVâÝ'?ueÿgu?ïû…+âK?F"…óíÌ?Aëß-G¡µ?F"…óíÌ?îvsM?²‰1Úëý?®h˜Éÿ¬¸?²‰1Úëý?îéÜ3r?™X•%=<§?¡b<ÌiCž?™X•%=<§?éQ~ÓÂõ?ªcŽïÂQ;?ʺ³˜ô-?ªcŽïÂQ;AGN3FGL J0349.2-1158@i<c>ÿPÀFÞ-ÿ틉À:.¶(E™gÀ;¤¬§"W`¿Ó7‹¼%#•@Qð/¨d8?ûÀ
ÿ±¿äW̍ÀP¿Ã1®õ\Ÿ$?¼~=Ù»ƒà¿Ø䢃šv0AGNbll@²¨ÁG®{PowerLaw1ES 0347-121?ïÿ}N½ÛÌ?àP¸Hü.?V#Hb?àP¸Hü.?ïҏâ`²È?‹ýD>k_?v¸¸ù0?‹ýD>k_?ïë:ýh1S?Q⤯B?dÅ̼È?Q⤯B?ïþ<ŒUìÏ?F2i_ë?,78^Û6ô?F2i_ë?ïÿhÊÞ?Œ‰ôþx5?,VV@+ÿ?Œ‰ôþx5?ïIÌ­OÓ?¯?«!‡P?–Æj^ÍÓ£?¯?«!‡P?ïè®M8u›?lAÎslfŒ?gQ²ôå<×?lAÎslfŒ?ïù¡ûy×?BúÎÁ³j?Ix%Þü‰?BúÎÁ³jAGN3FGL J0349.9-2102@jÌ¡ á÷×ÀHƒ-••À8ÅQa£ÊÀ;Ÿ>øcSŒ?û¨:üÖ)î@í-(­Z@Þé	nh¾¿àzZá;Þl¿èù›âÊ¿ëòPË°©<¿ïù¤ë¡#AGNfsrq@xº^5?}LogParabolaPKS 0347-211?ïèéÄ»lŽ?q8q;y¤A?g;~LáV?q8q;y¤A?ïÊÉíŸUE?‡`SLº5?z›	×=k?‡`SLº5?íŽ}Qœ?¡‰Ü3mC?³ŒeåF?¡‰Ü3mC?ï¢iƒ@*¬?o¸My.Žå?‡eŸ"6å?o¸My.Žå?ïǙ½
ù?}Y¢ˆS"³?|3yëž?}Y¢ˆS"³?ï·Þ§Ý?¯n{6@ԓ?œI5+Ì[?¯n{6@ԓ?íè­Eîé?£¹¯*þÆ?°º•Óìo¸?£¹¯*þÆ?ï"²@?éwl6ù«?›©¾~ .ƒ?éwl6ù«AGN3FGL J0351.1+0128@g[@îÙÀCÍÿÒ³—À:qbBë7À;‡»DLÊ¿r4G9b
@
›mrÊ!ø@r*ßý ¿â®õ惿éì¸
Ú
¿îùW'8&b?éM°&±AGNssrq@@c¼ÓZ†PowerLawTXS 0348+013?ïýôG:&B?=½Ë*ŽIú?0]Æéíu?=½Ë*ŽIú?ïÒGwìS??!V{‡—?vô\AúW??!V{‡—?ï™c–}Zt?~UÙ½?‰§VZ?~UÙ½?ïÿyj°?Ç&°»§?ÝùÒúð?Ç&°»§?ïôÜ_ß0?`G×ù/e?VG@&"ãâ?`G×ù/e?ïAd*'y?«î拼k"?—Ó}×KtÖ?«î拼k"?îj7g†ˆ?ž••>pG?§)\ˆ«°~?ž••>pG?ï梨ñ²	?m;,ŽÄÍ|?`X]Bˆ:?m;,ŽÄÍ|AGN3FGL J0352.9+5655@b9ø -à@½¾`Mr¥À9¿aY·+{À;j¥.ùÏ?è
~A4¹×@
ßôA…ÜM?ýT@ÿ¤n?é_{Ò£[?ïú¼3Cñ"¿â2	6¬Üº¿Ù£}`Ül[AGNbcu@¶°¶_Ø­¬PowerLawGB6 J0353+5654?ïúeJÌEØ?PŒ]"GO?FjÔÀrò?PŒ]"GO?îÕÐÉ~6?¨rúQª?¢¢óhû" ?¨rúQª?ï‰GsJê#?Š±à‹'0N?®#7"K9?Š±à‹'0N?î@nîRâ?'íkbUˆé?«ù>*×?'íkbUˆé?ïÖÖTÏ©æ?wï×DzEµ?t"Õ²H?wï×DzEµ?ê]BM­\ð?È°ñôha?ƊöÉJŒ@?È°ñôha?ï"Áœyb?"Ë-1ÞÁ¹?›§Ýő›Ô?"Ë-1ÞÁ¹?çëž7–£?¿HŸQòï?Ð)ðÐҺ?¿HŸQòïAGN3FGL J0353.0-3622@mÄô@¯¹ÀIUøØþ3À:w™Á݅'À;®0Ô´!Û?¶aš
¸	@Ì<C¨ p?øÚu!??Ü¿ïÿVëQж?ïýÍ«øty¿ÐGЬ³ÛB¿Ê'H/wDŽAGNbll@¼C'òäPowerLawXRS J0353-3623?ïÿ[¢4•*?	È×Aj?‹¶Ïø»O?	È×Aj?ïÑQ"
?Ž`Ý?ªŸ?wu×%Híb?Ž`Ý?ªŸ?ïà ÙT?r¾®-§¼?oß'$'˜È?r¾®-§¼?ïú"ß<ÞO?1Κ©‰ïD?E°'—új~?1Κ©‰ïD?ïÿ<ˆòW?÷ÆÙ)¢?rë?‹ª?÷ÆÙ)¢?ïZ¼ºŽX?ªÆ¢fFÛÝ?"¨hª¾y?ªÆ¢fFÛÝ?ïã¹%®˜ã?syi]ô ?lFÚ>)MX?syi]ô ?ïè[…P¦%?\ô:¦L`þ?g¤z´Ù;r?\ô:¦L`þAGN3FGL J0353.0-6831@q¬' ÄeÀDcX R…ßÀ:;Äõgö‰À;­…¨K
E?°QÔ
°g@
èlXï
?ùÑ°Ÿ¶5¿ã?^…zˆ¿Ýå‰ïNú0¿àì7¶(¢?¢¨´"œ¯¤AGNbll@ÀU'n—PPowerLawPKS 0352-686?ïÿöÁ	m?ªÔ¿»c±?á!cÅ5?ªÔ¿»c±?ïÓºd•Uè?Ž¬}¿ ü?v"͞§ ?Ž¬}¿ ü?ïÜË~ÝÅ\?tÐq¨©ùÙ?qš@–œ±Ë?tÐq¨©ùÙ?ïüŸY2\…?,¯ixÑ©?;4Q?¢ñ?,¯ixÑ©?ïþ-åÀ0?(ž^îþ›?-'ށXAÏ?(ž^îþ›?ï.¬ƒV6C?°zՄzzO?š*oŽYÿ¹?°zՄzzO?ïÒĂGæ?|¡klÑ?výªîQ<?|¡klÑ?ïÚXŽêò…?na2îìf®?rÓ¸…·Ia?na2îìf®AGN3FGL J0354.1+4643@cGŸfb5À«
–ìÀ9·ß(ë²À;Y
W—Õ¿'ÙK•'"f@iÆ@ì"M@
ä?Z2ü¿â'¸…¼Ì¿çÏNK+f¿â¶ë±`Ø¿æSZ¨m
AGNbcu@öíà
qPowerLawB3 0350+465?ïþµá"?*¡á%£¿?$¡í†:]?*¡á%£¿?ïžK¤»ƒ?—Ö=‡÷?ˆmÛn
??—Ö=‡÷?ïã4"ì—ª?cÅÂÐË8;?lËl%FNW?cÅÂÐË8;?ïé~í#?K3V"‰2?fì?K3V"‰2?ï÷¨Ãƒ"	?Sc¡G0hÅ?P®y-õýå?Sc¡G0hÅ?íèµlø•—?¸›"燘?°ºT™…-Ä?¸›"燘?ïqT†jí?ä3X¸w?'Õo+ފw?ä3X¸w?ïÎÀö]?ˆ?Eõ‰'Á?œ¼¦'á4R?ˆ?Eõ‰'ÁAGN3FGL J0354.6+8011@`Lþ?5Ÿõ@4¥_ yˆÀ9†mpEã9À;ٞÞ|øy¿âùͶט@Ld×pä@ü?_'`¿åÝë«_>Õ¿ä>ñ5'g¿äN­i"¿é ä´AGNbll@Š¶c¢œwšPowerLawS5 0346+80?ïÿ?Åà÷?mœ	,?E¿,©ˆ?mœ	,?ïÕÙ©‡«ä?†v‹-¸Mx?u+=‰æ?†v‹-¸Mx?ïÜî3Q3?v[ øŸÑ?qˆ¹m抩?v[ øŸÑ?ïÿön³^>Æ¡ˆLúi>ÓÍC¾SoÍ>Æ¡ˆLúi?ïÿ0Õ4û4?ǎ´Nš<?å[òŒ?ǎ´Nš<?ï¿"]£'?°0h{?œh
k´•/?°0h{?ï·ê.©Øù?"¤do‰"?'tb@O›?"¤do‰"?ïÿ̞ 3t>û¦i_I=¼>ù°â±[,>û¦i_I=¼AGN3FGL J0356.3-6948@q¿÷À*ýÛÀCéUÿæՍÀ:C|»<'À;ßÀãŠ~tÀlÌìW@U<µ'ôd@<šà–ƒ:¿èúJÉÒÇc¿×Ù­w"œ¿ïÿ׶µ´,?ï÷7ã=ŸAGNbcu@"ü*™0¾PowerLawPMN J0357-6948?ïûþ-õ?I]õªï³Ô?@ˆÌ‡´"?I]õªï³Ô?ï×Ëú™Ç?"Öx¶äÇÚ?tÐ$:?"Öx¶äÇÚ?ïW®Q§?‰ö5ž>ç>?•
=d5?‰ö5ž>ç>?ïÿÿö߉­>Vê
qcg>Qó@ÀƒÂi>Vê
qcg?ï𮞛?f^VÛ*žê?^¢Ä±ú\?f^VÛ*žê?ïJn
Ÿ–3?®üÏ;?…Í?–²>¥.®?®üÏ;?…Í?îOê\Ö_?%ÊÛ'?«^?%ÊÛ'?ïÿüŸؑ>Ԁ'$eÙ1>»ëlE²6>Ԁ'$eÙ1AGN3FGL J0357.1+2325@ehß½jYÀ6ppCßÀ9ü³1ñÔÀ;˜Ûmy€¿ß>^Κ@
¦•°ÖÍ@JÀŒ}¿äÆî–Ì	Ù¿ì—Õ°\¿Í™Sƒ_Æd¿Þ='7äYAGNbcu@'™'@·€4PowerLawMG3 J035721+2319?ïÿ#í×¾?#cìÿ'Ý?'=ÿý°š?#cìÿ'Ý?ïÍ)&ûþz?ŽÔþ•3èÂ?ykl"Ž¦ü?ŽÔþ•3èÂ?ïàcSÄ?c²õ&…jV?o~œº¡¬,?c²õ&…jV?ïýv~ș?"ŸÚA,Šr?4L	·ê­Î?"ŸÚA,Šr?ïýшãÜ?6ø>k?1sºHâ•È?6ø>k?ïžÄ·æ?°†¤kd?Ì'gK^e?°†¤kd?ï¢÷bŸ:?ƒœ¬d³j?‡B8cè•}?ƒœ¬d³j?ïì¾9ƒ|?Yَ]1p?cæAÖú¤'?Yَ]1pAGN3FGL J0357.1-4957@p+i€,
JÀHb`GhtÀ:+à¤&À;ù)CÆ(nÀE¦}X@V†´åzn@DŽ*GQ¿Ý!Œ@hâ¿åwºXáA¿Ù¤ZŽ}¿à¬$vAGNbll@šÑ-à
qPowerLawPKS 0355-500?ïÿ¶í΋O>÷vdàÁ›
?D™'ŽØ>÷vdàÁ›
?ï×ÄzÌW?ˆyj€ûˆº?t™Ô87?ˆyj€ûˆº?ïð4³v8?L^òöúj6?_–šrDއ?L^òöúj6?ïÿþz;QÝ>§‰XL ê>¨Xü+ï
ý>§‰XL ê?ïÿÍKˆû£>õE¤ÖÐsâ>ùZAÙðÏ9>õE¤ÖÐsâ?ïB8 Ê)H?±EªG"qÊ?—¸ëê*rô?±EªG"qÊ?ïír""+?gT£FƒU?bÞ*eTÔ?gT£FƒU?ïÿÚtïÚÞ>ø&X6¥Öà>òŒ\
>ø&X6¥ÖàAGN3FGL J0357.9+3206@dX6m
JÀ/ù£~õ©eÀ7q=Y&ãÀ;="Ö¼@üFØ
@ñˆ\…g@"Bè\ö¿ÒJÿ5]c¿ã(vÛmhR¿ì§nœJW¿ïj?©¹!tPSRPSR@c& YŸPLExpCutoffLAT PSR J0357+3205?ZÔÆ©¶b?dQ¼œ¼+?ïò•œ'zõ?dQ¼œ¼+?§fök?¾xªûZ˜—?îŽùžx6Ú?¾xªûZ˜—?ªˆýno
C?Ÿ'zs93?îWp(ÔVü?Ÿ'zs93?/ߘ®ØÅ? û!Ùm·?ïþj}L? û!Ùm·?L=B¦®Šá?M™È؀¶j?ïøð¯U´?M™È؀¶j?•¼¶Y#û?²–]¹&yR?ïRúh³À?²–]¹&yR?p,&¾I–?‹-´<^àH?ï|~žÊ
³?‹-´<^àH>ù‰d'ì‰>õµóg¹nú?ïÿÌí•*…>õµóg¹núPSR3FGL J0358.7+0633@fê}æOUÀ@Çk 	ŠÃÀ9EçbzH›À;s® 9[k?Ütëüà2R@ØJl4܁@É •¿ãþÚ®ŒÅÌ¿é9Y¤e£¿ãu5ÀØß¿ïÿqtâUAGNbcu@l ě¥ãPowerLawPMN J0358+0629?ïÿk€+´d?ù»w׆#?µš¥?ù»w׆#?ïÈ9*,?uÆDŒ:Ð?{üãd±Ñ?uÆDŒ:Ð?ï§ä½{Ãg?xs?†ГP¶C?xs?ïÑð"a­?VÿCÏÞ<?wu"¢ý"?VÿCÏÞ<?ïÿ¬ìeL??RqO?ÄäÊô²˜??RqO?îôžþ»åÒ?³è"ÍÕlv? ¶‰ÔÜ?³è"ÍÕlv?ﵤÔ$Û?âû{œ?'–Êè27B?âû{œ?îóϽdqf?Œ`›(îi]? Ã+p·œ?Œ`›(îi]AGN3FGL J0358.8+6002@bàP7P@è‡@%´ðÀ9…З]À;Nâ~ú?Ý3ÑÏÒ!@)ðÐq@$ˆÿÃo+¿ãØÑÂ؃¿è²‰"p	¿ã‹·	RJa¿îXQúøÄAGNfsrq@ƒHÝá\¦ÊPowerLawTXS 0354+599?ïüî"æg†?1arw?8ŽéÕ¿FÜ?1arw?ï¼¹"»¹?:û;—?€Ñ·Z±9¼?:û;—?ï`8Ä—³?‡†,ô7œe?"øçv¶¡?‡†,ô7œe?ï÷ÄÿgÃw?3µºŠ¡˜?Pv˜í0t?3µºŠ¡˜?ïý~…ìéx?3'"c•`þ?4ÎõÊJ?3'"c•`þ?îoÏ@;ý?¸üó66?©#kÜ1?¸üó66?ï1‰›ár?"
}†©?™ÎßÊÌ´?"
}†©?ïß\êÅ8â?c6nO¯?pQŠ{·c?c6nO¯AGN3FGL J0359.3-2612@kØädIVÀH!'	±À:"QN"¹À;Û4̐fë?Ó½I¬ÇHÔ@
Y9Ìö@Œ4ÿf'&¿è‡-á7¿é£¤"ƒç¿Ó‰J†áÛþ¿æHðLÙ¢AGNbll@ ºg-PowerLawPKS 0357-264?ïþ©æeF£?P¡"o%U9?%a–yŒl?P¡"o%U9?ïоn+‡?'")d7@?w ÈÖ&Ìu?'")d7@?ïåñ©KØ?iŒ_ºÕ¶?jû`Sé?iŒ_ºÕ¶?ïÃ{'?aÕ\<e¼À?~B6üÙio?aÕ\<e¼À?ïÿnŒ>	?*¡æ'À?.t+*åJ?*¡æ'À?îó䧛 >?­`V8é"? Áµ"–.(?­`V8é"?ïË<*²?~ÂVá=*?zaêçÑL?~ÂVá=*?î]>'¿ò?š´ß2dˆ?ª,†¡åÛ?š´ß2dˆAGN3FGL J0401.4+2109@emÌÀ7"À7UH¿ŒrjÀ9˖‹È¿À;‹³ß•ý-?îjÌÌÒJ@á㇤N©@ω REr¿â½¨ë¿áŽ"Ç̀ô¿åœ,4ÖZ¿ïÿ4`tAGNfsrq@CwškP±PowerLawTXS 0358+210?â9é|Ÿ§"?Ðb×lGz?ی-À°×?Ðb×lGz?áy•Ä31l?Êö£í§Û?ÝÔw™(?Êö£í§Û?êÚ Í=?«ßäܬ÷l?ĕ|ËÏï?«ßäܬ÷l?ã"ÜH?à?¥R?VÒY?ÙðöGo€A?¥R?VÒY?Çvüéæõ?Ǻ!ÀUVZ?ê"OņC?Ǻ!ÀUVZ?ÄÏОy¹f?Êñ.Ô`â?êÌØa'§?Êñ.Ô`â?ފs_âØl?¾ö:Õû?àºÆP"Ê?¾ö:Õû?»©Òqؾ?™Ó¿¬¿s?ìŠÅ°Äè?™Ó¿¬¿sMIXED3FGL J0401.8-3144@lå7?1n7ÀHN‡à3±ÞÀ:V"ú¾À;ò·1Z?²åäÃ0
[@}ù?œx@J‡™xb¿è"Ûs¿çÔÔxñ6¿Ö¢}›Ǩ¿ë-:¾AïAGNfsrq@†•à¿]xPowerLawPKS 0400-319?ïý֝0'?,%‹:3X?1KH-[?,%‹:3X?ï;"Š"Â?â*ú¥Y?y ½¹VFâ?â*ú¥Y?ï­'O'i?xhk¦¥œ`?"¶,Hô•³?xhk¦¥œ`?ïÍebå?^‰jÝ?yMwA~õ.?^‰jÝ?ïý'¯<?4Á°ÿ6•<?3ꁴŠÔ?4Á°ÿ6•<?ï>o?±!¬Žì?ŸX?·D=?±!¬Žì?ïŸo´+t?ƒ±ÕDQ}ö?ˆ$<`³'ø?ƒ±ÕDQ}ö?îjzc.´°?˜ô®GŽz{?©XYÉ¥?˜ô®GŽz{AGN3FGL J0402.1-2618@kä}sÉÀGÓõÀjÀ9ø|]H°À;·ßâSG?åËWw"½ë@‡õ!ªŸ¦@ðX•m?ï2î>âi¿Üc‰¨ÆïN¿çÛ¸M
û¿Þ¿9€:‰AGNbll@Ÿ)¥ýŠÚºPowerLawPKS 0359-264?ïü¸:¢û?;ôX&£?:>)à­O€?;ôX&£?ﺢÀß®§?…žÉ¹"áö?WOÌãÊH?…žÉ¹"áö?ïŒÅ±z6?'l ¢c?ŒÎ¾ã"?'l ¢c?ï‹u®F¿?Òaj2ãª?žŽ'Kîö*?Òaj2ãª?ïòþwF§?]c<9½ù?Z¯@ß?]c<9½ù?î±5"Ÿ?¹9Öý‡'¡?¯쥏"?¹9Öý‡'¡?î›î=éM??¡n¶RH3?¦A%¶¯?¡n¶RH3?é}§ŠöÈ?µÏVo"d'?Ê	a×Ð$à?µÏVo"d'AGN3FGL J0403.7-2442@kž¤_ZÙjÀGzX`fÀ:'ÅÁ?ÐÐÀ;ö2 f<u?¼#$Œ;j@ñÈS{½@ò`À48¿¾–û\_Û¿ë¡ÃBE°õ¿ÞýϦ=cZ¿ïòÂómAGNfsrq@'(†YJôñPowerLawTXS 0401-248?ïí&Æ,8‡?bjx?(?bÙ:` ²?bjx?(?ï¼×!ö†?¤Êf`Ê?€Ê7wÄÖ?¤Êf`Ê?í²¿2¸íz?ž't­d?²jk'n«?ž't­d?ï*)Roõ˜?š§/R?šºÕ²M?š§/R?ïìÜìÌéË?iUr'ƒµS?c#pï-)?iUr'ƒµS?íš~'*ŠB?¹bk"‰.?³,wõˆl?¹bk"‰.?íöƒ]0÷?¡qØt»
?°O䨄Æ?¡qØt»
?è;µ*wU?¸"&ôò–ò?Ï…+V"ª?¸"&ôò–òAGN3FGL J0403.9-3604@m·{€©Þ‹ÀH;Ã`<€ºÀ7/.g˜À;>K֘'ª@Žƒ¹Þ^@FG¤5)@¬BIхC¿â¡w¾ji¿è ×ÌOñ¿êPEҔ"S¿íÈ%?¡øÛAGNFSRQ@rbb˧3LogParabolaPKS 0402-362?ïê t ?eŠ!U‰û?eߋÉ%é?eŠ!U‰û?ïÒN-¬ØÞ?‰jâˆ1"ž?vØé-³?‰jâˆ1"ž?éôXÆ%úÍ?¯;ý˜®?È.œçhÍ?¯;ý˜®?ïîˆImºÌ?S²ZrÁ?aw¶¨B³À?S²ZrÁ?ïÚûã…‹?p7ñл"?r'#`'¤?p7ñл"?ï[\|ؘ³?¬A4¶gœ?""pf¤· ?¬A4¶gœ?îH;®?¢B•JÜE†?®ž«´»ë?¢B•JÜE†?ïòR!­FA?ZVµDÎË?[[¼ªòÝ°?ZVµDÎËAGN3FGL J0405.5-1307@i¸ߨq¤ÀER3çüÔÀ9Æ$PA`óÀ;Èi;,ü¸¿ô/Þr¾"@öÉ™"{@Ä<€L¿âËK-ƒyz¿æŸÚ÷e…I¿áa¯Ü7_#¿å³` åÏcAGNfsrq@‹Ì':)ÇzPowerLawPKS 0403-13?ïÿì?}>â:3"õD>ã~ÙQ]w;>â:3"õD?ïКÊú˜@?"«‡m?w²šyø5?"«‡m?ïô´À;™ß?D|ºý7)M?V–FÓÂ>?D|ºý7)M?ïÿè$Žw>ޝµï¥v>çÛ::°ô>ޝµï¥v?ïÿì*F`É>áP8I1†>ãÕ¨¡¹^R>áP8I1†?ïL—]TCú?®'Qù<á?–mPPÇ?®'Qù<á?ïì™^"ç²?dîrKd?cf¡/Ÿ.Ì?dîrKd?ïþÿ­}YÑ?^
áPw? +ñôò)?^
áPwAGN3FGL J0407.1-3825@n(*Á	J,ÀGìè_ÐJ0À8î÷™ÿñÀ; ÓµZ?ð¡R¥ê4è@õ5`Šz@.âôV¿âŸaþü¿æ=U?;n¿åp»ÝøTv¿ë ÂJñIAGNfsrq@"JÙb¶®PowerLawPKS 0405-385?ïú)O?CÑzò®ý?G߆z§¥?CÑzò®ý?ïÎ[†þ%N?ˆ3*U½A'?xÒ<—šÄÈ?ˆ3*U½A'?ïxcCqCå?"›µV"F]?ó—–þíX?"›µV"F]?ïÈíu‹?_ a@®@?{‰E†˜p/?_ a@®@?ïõ¥ˆ€?SD0^ªã?Tµô¸Õ?SD0^ªã?ïš=a?°^Dv½?œl¸WMXs?°^Dv½?ï3+¡"ö?'ÓՉp?™š‹ÖIW?'ÓՉp?ï9~ô¸à?†ÓD{©u?˜ÎÑÞ?†ÓD{©uAGN3FGL J0407.5+0740@fý-`ûHÀ?)£?4É5À9\¨\ªûÂÀ;nNá£1¿ñÕ«}Ç«ü@Dõvºš@…¹'!*¿è®+£4I¿æ…Œ™"r¾¿ë^BØ¿À[{26šAGNbll@'­=!ÿ.IPowerLawTXS 0404+075?ïûb$Ét9?LU©"–?BwlD¦ƒi?LU©"–?ïÔãv~ÙÇ?'Ëf×`µ´?uŽDÝoÔD?'Ëf×`µ´?ïf#ÿtÐô?‹Ò÷øäF«?";€
öE"?‹Ò÷øäF«?ïÿ¨Ï	>ýs[Ïδ?ÌFÅëÒs>ýs[Ïδ?ïäê$³Ð?p©³uY?kü²à'?p©³uY?ïT꾂å¬?«È¥;ºö?•b¨-ë|?«È¥;ºö?î\ÿ¸â?ž›MX5f¸?ª0#¢ÊÚ?ž›MX5f¸?ïõP"ÛO$?Tá•'&w?U^öT`w‹?Tá•'&wAGN3FGL J0409.4+3158@d–]¿Î·‰À,ÎRAtÀ9ÿ°ŸoœÀ;‡yÎøö÷À¢ëý¿‰@S¿[o'@û¨»w¿êX™|ÆØ ¿èžô'%Æ¿ÓN¦Œ-¿ã‹Õe"¼AGNbcu@"Œß!-w2PowerLawNVSS J040928+320245?ïþá‹
?$T×`FÊ?!¢'K?$T×`FÊ?ïÎDég–?…ìªÍCv??xÝÿšj}	?…ìªÍCv??ïÖdf9£m?lº \ÑÇ?tÍÌÚï9[?lº \ÑÇ?ïÿÿ\Aƒ>"ƒƒèX>"xǨk>"ƒƒèX?ïüšQÇÀ@?<«Üµøž?;-r»"Òi?<«Üµøž?îýÝÓ|¶¬?±X¯ÂÆ{´? ""ÇX®=?±X¯ÂÆ{´?ïz'F$bÇ?ŠW/Æÿô»?­·BRß?ŠW/Æÿô»?ïÿì¿
u>èø0ßÇ#ù>ã=÷,Ôö>èø0ßÇ#ùAGN3FGL J0409.8-0358@h{¢ÿ‰;ÀB¯Ø€_5ðÀ9n93't¹À;‡#µîe?ë\˜1e@WtßP)@"< DXŸ¿ÅéÊ A‹]¿àuñ—ë¿âÏòU¿Çx¿àŽ¬£ŒŒ–AGNbll@š
g8~PowerLawNVSS J040946-040003?ïôÌëõ\?Z‰óôÚä?VgֈJW`?Z‰óôÚä?ï»·¨Å¨ä?Š¯ïðÖÎ?ׄÃ?Š¯ïðÖÎ?ï´}tä?~¸Îìy?'û`š‡È¼?~¸Îìy?ï%†0u¤?rQ9Hý?›O9ö‡5ˆ?rQ9Hý?ïì«$	%?\¸HÞü‡H?cTÛCœÉ?\¸HÞü‡H?î3C±'!N?µæ"WÝ{`?¬ËÄíë?µæ"WÝ{`?îfÙ
!ü?¢5znі?©'o,(j?¢5znі?ë¶mÃZ'?£¦€kvûÈ?á&Hò•½?£¦€kvûÈAGN3FGL J0413.6-5334@pm#@ˆÊÀFR ÿ¿h`À9:mæÎÀ;¼À2Š–Ç?ÒGp²D¶=@¹Zîu@Ïâ_[/Q¿ä"9¿äEÕwŽà¿éH0s˜ÜŽ¿Â‰,2§¶ØAGNfsrq@Œ¶œ]cˆfPowerLawPMN J0413-5332@?ïÿj{ÉÏí?"½Ö¸î?°®Eú?"½Ö¸î?ïÌê©×X?'°ó8­¿?yŠ«2|ã®?'°ó8­¿?ïÒw¤¯ÕÏ?pc*X®kÝ?vÄ-¦Tª?pc*X®kÝ?ïÿ¨'ѽ3>ô×w>ùôì?ßLÞˆ¼>ô×w>ùôì?ïþåL0ÁO?""¯Ä'³Š?!«:÷ñ'?""¯Ä'³Š?ï[O:6û?©øºH]3Y?"–·…2œ?©øºH]3Y?ïd'Ǭ8?‡³t9¢]ï?o¬1ã?‡³t9¢]ï?ïþOþ3æÑ?%ÖB¥åÐ?+¶	¶È?%ÖB¥åÐAGN3FGL J0416.6-1850@jÉ{¼¾bÀE/0ŸÚü:À8þ,"	7À;«kÙlî@¿¬=¨7•c@Á'eé>@¸áß®{Ô¿ä€ÚB×%¿ã
–t 8Z¿è_
Úyˆ­¿áEÀDbDAGNfsrq@†¾vÈ´9PowerLawPKS 0414-189?ïÿxâ{?%opuö?ã´BÃ2a?%opuö?ïØH¸«ƒ?Š¢hƒ•?sùÛ²š™?Š¢hƒ•?ï͏ßþÐ"?r'ùJ"Š ?y8î¹÷R?r'ùJ"Š ?ïýÚägž?2Ý
Šü?1(ÜÙˆ¾?2Ý
Šü?ïýTtÔñ½?7µ"ѕµÎ?5\Z~éÍ?7µ"ѕµÎ?ï6Ìç
 ü?²ý®ËgÄv?™&cܨ~?²ý®ËgÄv?ïp¶Oݹ?‹åæZ"É?'ý)6Hå?‹åæZ"É?ïî²,Yò‡?UžGкrK?aMӘO	?UžGкrKAGN3FGL J0416.8+0104@gúŸDÔEÀ@"п "`À9‡Ûk=À;Wè°X"ÀþHDè<@0:/{Ä?ûë©ÿ˜Q?éW
¥—̿仝‰'&¿ÑmE;Q¿ÐàP7OøfAGNbll@´N¸>BZîPowerLaw1ES 0414+009?ïþöIa·š?н†ò%"? ›i…÷Š?н†ò%"?ïÔÛ±J?‹J'Q)Ö?uüqøº?B?‹J'Q)Ö?ïá3è ú?hz'£ŸA¥?nÿË÷ž;?hz'£ŸA¥?ïÿÿÞ¶Èî>tÜì|澐>p'˜'ë>tÜì|澐?ïþéŽ	Ô¦?"<ºí&üã?!g`'¨l?"<ºí&üã?ïhÀ+B"?©;W¦Ò^©?'þó¸u²?©;W¦Ò^©?ïÖ­Çà0?xØ+æèË¿?t©üº˜?xØ+æèË¿?ïÿþ4ù±Ý>³Ds"aö[>¬³UžÂO£>³Ds"aö[AGN3FGL J0418.0-0251@h€§ayWÀA"@f!À9#'RÑ^À;‡JaM!ò?ïÇã_û,@=×{ýQz@¯'ÿÏ-¥¿ç'üÏ¿áçй–d0¿épN[$O¿ïÿݹë.ôAGNbcu@ˆ •L˜_PowerLawPKS B0415-029?ïñc£¤›'?`lþ°ŠÌ?]8¸5—º?`lþ°ŠÌ?ï­¥O«?ˆ‹(ôˆ+?"¿¹|yR?ˆ‹(ôˆ+?íi˟"õ	?¡ê×½«A™?´±£4>·?¡ê×½«A™?.̖?€éþ­5Õê?¦-'O©?€éþ­5Õê?ïâ†Õ>,Ù?{x'ߨ^?my*©÷Z?{x'ߨ^?îœ{~Ú?³Oi¬üSÌ?¯8IÊ-É?³Oi¬üSÌ?ëߕí»¿?©X3QHïs?À¨K¹?©X3QHïs?è'ÞŠô?¯´ú·Ûh?͸‡÷ÁÔ2?¯´ú·ÛhAGN3FGL J0418.5+3813c@d2`c'À!N·@§[À8סíûñ~À;4'b"s?ð`ãD³c@Ðü&Å£@K7GMœ¿çՆGqD¿ëùt7	'¿èˆ¦0š–^¿ïÿÒ"¢kAGNrdg@r2þÅm]PowerLaw3C 111 ?ïÙ
'\?z¨‡ÈÁÔ?sy7^D
¶?z¨‡ÈÁÔ?éöò\FÝ?Â#ù!Q?È$6¢ä‹?Â#ù!Q?îì0%j#?'Ôgd¬ì¡?¡<ý«IÁÖ?'Ôgd¬ì¡?é;¼8wb/? $Bë?Ë"wF? $Bë?ï2åa‡ô?¡×óSk¯H?™£SÈ"DÙ?¡×óSk¯H?ÔÍŠn)?ЃÂ(Wa?å™sºÈúk?ЃÂ(Wa?齅Ôëª3?µ°e&	#÷?É	è¬QW6?µ°e&	#÷?ÑlHß"?¨Ÿ]³ýW‹?çIÛùz6?¨Ÿ]³ýW‹MIXED3FGL J0422.1-0642@i@lÚÀBÛíöéÀ9®°E­‰À;¹V¢¤W?易 ûðs@Õ˒@Q†Àyt¿àÖ.½Ø"*¿æ){þS-¿è§´í]&¿äj"]Ú£AGNfsrq@‡
ˆ1&éyPowerLawPMN J0422-0643?ïú¤‹åüÊ?añá×eu?EmÐ<Ùê?añá×eu?ïžûbÁ?'{-¼´xY?ˆAU7³Ù?'{-¼´xY?"âr?"*œÀNfü?ˆšÊÓ¾?"*œÀNfü?î¾@ڈµ?€÷¼"§=%?¤òV¢¯?€÷¼"§=%?ïÃ6dQI…?‡÷Óbrxß?~dÍî©k?‡÷Óbrxß?ìˆ*óµß?¼à[	ø`?»¾¯0bQ?¼à[	ø`?í´yÜ\Y??§ìöfc?²\16?§ìöfc?å°!˜¬Ý?µnõ¦ì°›?ԟ¼Î§îF?µnõ¦ì°›AGN3FGL J0423.2-0119@hi#ßm¹AÀ@5ߵݝÀ7‹@ºs,À:îﲪâ—?õºX€õ‰@%@ô¼Õß@ž`‡)T¿á×ù}Ò59¿åwGø<<F¿äÝÌ_¥¾&¿åÃ'Š¼ÂAGNFSRQ@©aùðLogParabolaPKS 0420-01?ïÿ
æÍ#?ÐÅ6?G‡†^Êg?ÐÅ6?ï܈ùR*´?'è{².?q»ƒjØaé?'è{².?ïÒ5!Óm?p‡±ßfz"?våo(¶¬?p‡±ßfz"?ïö§Mü?:–KÄá?SÀ²6šX?:–KÄá?ïþŔ•w?*ÓÉKœÊ?#¦Áû3V'?*ÓÉKœÊ?ï;T!óÎL?°'0›çJ?˜•{º¦þ‰?°'0›çJ?ï̏øéò?€eµ³Íï¯?y¸~u̖ä?€eµ³Íï¯?ïï Kœ?Tàx̪ž?`ë_q™8?Tàx̪žAGN3FGL J0423.8+4150@cöX@žUÁÀÃßé47À8MQŒ»À:Ú¥ÉRÄÉ?áE9bã@«ØW—V?þC‡¿&›ö¿ä™˜¦eÁ¿ÞãÙ5¿ÌOąÍ×0¿áS#h¹0AGNbll@¤¾=cˆe•PowerLaw4C +41.11?ïù6cO–Ò?CYuçá`?K&sèc?CYuçá`?ï}Q]ƒ?–™Têþò?Ußy…y'?–™Têþò?ï1šDw½?–¾X?Ý?™Ì·†ÈU?–¾X?Ý?ïX€ôu÷î?zuÃ,æ??"ïát°žF?zuÃ,æ??ïƼa?x
)甀(?~<¡ÚzqK?x
)甀(?ì8Æv?Áý_éÁòv?¿6?ñÌO?Áý_éÁòv?î†î§úÁ?Ÿ@L_úÈ{?§'~¦Õë?Ÿ@L_úÈ{?ì¯D
 ýf?¦¡Š,q×?º…ß'øÏ?¦¡Š,q×AGN3FGL J0424.7+0035@h2¢iÀ?Ëy`>.9À8'Ld\¡À;Iû_‡O?ÑïdöyÄ@üŠOú"0@•?æ¿Þu—''¿åsÿ©÷h_¿àSwa¥%¿ë/ó
åAGNbll@'¥òGE8ïPowerLawPKS 0422+00?ïþÚpÏK?60¯u<?"XöøDA?60¯u<?ïÏ£›â?d*Tšê…?x.2€ûO?d*Tšê…?ï€á²•œ'?‰!tÛ#p«?Ç"dç¯S?‰!tÛ#p«?ïèJô'[?OD¹ñevê?gµ'ô"?OD¹ñevê?ïýÊ©Ž†?1a"^àb?1ªµ
+×
?1a"^àb?ïÁ.&?²7lýÕ'?žÚ9ÓӀ?²7lýÕ'?îЍMÓ>ù?š‰¾nàêX?¢÷+!ð)n?š‰¾nàêX?ï}ûéùa?~ÓæhŸ'?@'ÅûH÷?~ÓæhŸ'AGN3FGL J0425.0-5331@pbâ:¸cÀE€ÇßþùÀ9gCÁðÀ;ԝñ.ñ¿õåØõ$.Þ@Ùð5²"g@®ˆ  ^…¿ä¾è$/ùÝ¿äÔ7r2!¿ÜÛpí0£¿ëãAÄלAGNbll@Œ‰»~ÿ—PowerLawPMN J0425-5331?ïíÞºàç?adÜÒ?.¿?b!D÷=}&?adÜÒ?.¿?ï×I~ŠZÉ?ˆBnñl—Â?t[@Äqƒ®?ˆBnñl—Â?ï+!Ê]º?‡ŦªÞ—?Œµ7"GÉc?‡ŦªÞ—?ïÿ'‹R?À×2G?A¢Óã×?À×2G?ïçÁÉþ*,?kë$3Œu?h>67o»ù?kë$3Œu?ïPÈÞg
?°''*08?•æä9Ë´¼?°''*08?îPEºkÕ? ÖiüÅyL?ªû¤YCƲ? ÖiüÅyL?ïùñòn?H
U5DÄÙ?Kµ¿û½*	?H
U5DÄÙAGN3FGL J0425.2+6319@búâ~@#…ïÕ"\À9Â*·c®üÀ;röq?Ù¾9½w*•@Ì~ ïÏ0?ÿme¾Ë­=¿ã—vå˲'¿èç	<Gaœ¿Üf9±~N¿…è¨(0ScAGNbcu@´ôçü¹#£PowerLaw1RXS J042523.0+632016?ïþê>!β?#¶@ؘ?!\ ŒÇ_	?#¶@ؘ?ïÇ9—ü5›?‰â­Àµ?Ò?|c4ãòe?‰â­Àµ?Ò?ïéRÙ¹Ð?eÿ–øyT?f­&=PHe?eÿ–øyT?ïö`cº[þ?>çFY`?S?8î<Â×?>çFY`?ïúã ©ÌJ?IN^
ИÌ?Ds|RQÌ?IN^
ИÌ?îÈöÌO¤X?²Â¼ó»Îù?£p"8rƒ?²Â¼ó»Îù?ïʘ¦Æ?€«õŒ%<?zû³ø
?€«õŒ%<?ï²ò…ÿ<?z
Ü®Œ…ã?ƒC^ͶnÌ?z
Ü®Œ…ãAGN3FGL J0426.3+6827@a"¦°)(@*°°|À9ǾZCBuÀ;£°Ôcš¿ñ·O,´@ '¯€@Ò@!¿ã1i¼¿è3©a|‹†¿â'7Ín)̿䈺›"=AGNbcu@Û'Zîc PowerLaw4C +68.05?ïÿmqP,ò?ÁxËR?QÛ¢¨¡?ÁxËR?ïѨ…˜?‡VZÜA?w+øÉÛKÛ?‡VZÜA?ïë3š­ž?U#)_ƒ¡?dÌà#Yáõ?U#)_ƒ¡?ïÿAWýÜ©?zTï}æ?ÕãÝJm?zTï}æ?ïþ¼›Ë?*nˆX}·Š?(5
¥°?*nˆX}·Š?ïʛ´{?²ÏŒö—"P?œF¬¡Y©?²ÏŒö—"P?ïÌ>y"ÈŸ?xc[Lµ?yàÃ[Ø@?xc[Lµ?ïñÅ×)?UãÁFaZ?\tQø!Ÿ?UãÁFaZAGN3FGL J0426.6+0459@gµq'lÀ<î™?׆dÀ9RöT…"À;T"K"bÑ?'Šò˜Ö~'@°Ü{š*@q1ßöö¿åxŸú쵿çê_5UÞj¿æDªøÍÂÒ¿é>!'}AGNbcu@…_ö"PowerLaw4C +04.15?ïüubhç?7kÕoÂ]n?<TëìE|?7kÕoÂ]n?ïÎ]	Š16? 8äôG?xÑ{'©•M? 8äôG?ïÐAy¥ü?yaØ~w?wßC2¶áÖ?yaØ~w?ïä¾HÙc?O†pùý?kA·Œõ?O†pùý?ïúˆ²@¯s?M8øu¼x?EÝ7Ó©Ô[?M8øu¼x?ï-›|¦Lc?©-œˆpÙ/?šLgÆ×£?©-œˆpÙ/?ï²Eѵ.?—+š§O?‰·L¨'??—+š§O?îç'@Ùå?Šš¾0•q?¡†Þª:"´?Šš¾0•qAGN3FGL J0427.3-3900@nEg!éBÀEöŽ€`ãpÀ8»rƒ«ËÀ;AHð3Ú"?æ"Uö_Jò@¿%oü^@`;»²¿áÿfyJˆ~¿éç±(Ó"¿çµ'"?W¿ïÿGýUçÏAGNbcu@9¡vÝ­PowerLawPMN J0427-3900?ïþ'´G<L?%–ŽŸsqW?'Ô½Ê-/æ?%–ŽŸsqW?ḯ"ˆ|?nˆQ{Pa?y¿|¹+]»?nˆQ{Pa?RÝ%?|ð9rï4!?Ž=Õ'Ùµ?|ð9rï4!?ïÓ@DúÂ?Xo
J\—Ë?v_݆"œ?Xo
J\—Ë?ïþÀÖ',?&Ž6#jé?#òž""?&Ž6#jé?ï»Êz?±i¹¤k??œ½èžÞ~°?±i¹¤k??ïaWw¾±?pÊѧV?"ܵçaÕ?pÊѧV?ï#ÄàÅ'?‰§ÄN?›ŸgeŸ)?‰§ÄNAGN3FGL J0428.6-3756@n‡?úÁÓÀEÏàaÕÀ6jˆû¼¤aÀ:3Ám9Í?ù˜ðN²»@õØ •ŒD?þe@å£]¿Ü},ÈØC¿áC,ú¨¿ßì>{¿äŠI2à
XAGNbll@†Î;Í5¨LogParabolaPKS 0426-380?ïî8"R?cñwǤÔ<?aÇî8ÓÁ>?cñwǤÔ<?ïÎã¶Pè?.ò*9?xŽ$¶¾å?.ò*9?í÷þÖN­?§Þ¤oc:?°@	M2–?§Þ¤oc:?ïÿÔë".>êÐ!ƒ6«>õŠ"œÂÌP>êÐ!ƒ6«?ïØ.»\ëq?zñÝÈ¥?sè¢1=óª?zñÝÈ¥?ïG)Õ«?¯ê 3:?—¼!¤'?¯ê 3:?îñÿüqw‰?z®¿=¡? à=4
k?z®¿=¡?ïÿíÞ6Îì>ãÂÂFt>â!Ñ=Ô&¦>ãÂÂFtAGN3FGL J0429.8+2843@eG¯ ×{|À*ôUÿøÀ9¹õÞ>YÀ;W'2ÂÊë?òÿÞÇöú@ZM{³Õ…?ÿiE pÝ¿ïœø¦ÅQ-?ít:!ín6¿ÛÏY*Nï¿ãf pMoõAGNbcu@­›Z^5?}PowerLawMG2 J042948+2843?ï⇛Y&&?nÔ	~Š?mxdÜZV?nÔ	~Š?î`4¤ˆœ-?­—‹€ùè?©üµ¶šV9?­—‹€ùè?ï-]åI¬ƒ?'ÒøÝbKn?šTCZ:©?'ÒøÝbKn?íwâb	?•¹#%2ºI?´@ï¾9B3?•¹#%2ºI?ﱀyÇk?"´àþÐ-"?ƒŸá®ÇƒV?"´àþÐ-"?èÇNÑk%?ÈW áóŒ?ÌâÄ»†Sl?ÈW áóŒ?ìñ՜mù?¦ÒªÈ›-Ñ?¸qSþ*¢?¦ÒªÈ›-Ñ?çúʶòðÎ?´ÄHÆÁ'?Ð
j'd?´ÄHÆÁ'AGN3FGL J0430.2-2508@kóóà7ÝÀD "?Åè­À:•mºîÀ;Ï¥·µ
"?²v_ÛA`œ@­•ÇÒçï@‹ïà"?¿Ï#.LË¿áR»<	N;¿ç¿oA+n¿áq'ÝëXAGNbll@–ñuŽ!–PowerLawPMN J0430-2507?ïÿ5dæ´?ÂïD±Çª?Scí&œœ?ÂïD±Çª?ïÖ}?ƒ`/Íórd?tô'7ñh?ƒ`/Íórd?ï¿qÌdáÆ?zEöëÂxæ?€#Œð€?zEöëÂxæ?ïóE"ß ?@+8º¦ÍC?YtÖ óñx?@+8º¦ÍC?ïþn@-Q?+ãòøŽ?)sÞæJ?+ãòøŽ?ïF»vkʲ?ªÖΣ#¡"?—('9eá¸?ªÖΣ#¡"?ï{w?Q¤?ŒpQÐýN?';
N?ŒpQÐýN?ï~Rã¨M?@¯Â¸e?5£˜#Œr?@¯Â¸eAGN3FGL J0430.5+1655@fxV[åÚÀ5ªKÀ9B«×‰¿1À;NaŸWH¼¿á®ÅÁHh@Ò&Œ'@6†@ €¿äêG‹H·Ä¿ìRþ]Ï¥+¿ÍéY¨ñXü¿ÛšÝl"AGNbcu@Žð$Ý/PowerLawMG1 J043022+1655?ïþêŸNB?#O¼]$ð?!V
ßõ3?#O¼]$ð?ïÈâ'>o?'©KaN?{Žñq0<³?'©KaN?ïí'Åór\?[ÆmÄû?bm:FG?[ÆmÄû?ïÿfÛl7?Šb—øâ ?$ž¯¨!$?Šb—øâ ?ïþ½ëÏ?+¶$Z9å?$/?OJ'Ü?+¶$Z9å?ï²LØ{?±l÷¢?R?œ)¶'"Œ˜?±l÷¢?R?ïÉö¸éÊ?ärI?{ûMKS?ärI?ïüŠSÚT?2´9ë£?;­f×AÖ?2´9ë£AGN3FGL J0431.6+7403@a``þG™@1\w·À9±{£aÀ;¿Á§ÕœÀfºó±h@
±Šî0×?ÿÐNI¿¾‡*…~sg¿ãš+Œ°a¿Ûf¿ÕÌ€¿Ú@`"ú¯oAGNbcu@¥¶¢MÒñªPowerLawGB6 J0431+7403?ïýIÏ#`¥?6bÙà ^?5±…$ac?6bÙà ^?ïÜ¢8µºH?€!úuÚQ5?q®ã­aì?€!úuÚQ5?ïÕ6¨*"‹?ra£äIá?ud¬
JÒr?ra£äIá?ïÿöúaŸF>Ò7ûE˜>Ò
ÿ`šµ>Ò7ûE˜?ï÷¦zÜÔ?VÊ8m»·?P³
‡X?VÊ8m»·?ï*
+8N6?¬1œd
é?š¾º'??¬1œd
é?ï ë"??†€ÎgCÀ?‡Å­?†€ÎgCÀ?ïÿšl°á?#p
wTE?¬²nIɎ?#p
wTEAGN3FGL J0433.1+3228@dûá`؇ìÀ$Þܾ²W×À9ôwa`m(À;ûý<a¿ÛM¹ë¸d$@eýua+?ÿ~5?|푿äq#mÑG¿Ö¸ŒÃпàDe°¼~¿ÊÛk‰n†ÏAGNbcu@¯Ø33333PowerLawNVSS J043307+322840?ïÿu}z?5*í‰Ñ?QZùá|+?5*í‰Ñ?ïÆ!³ë?Žó!¶Ž:ù?|ýïø??Žó!¶Ž:ù?ïà"Ujž7?téjšÜv?okª Øß?téjšÜv?ïþóø#¬q?ìŒ? À©/?ìŒ?ïþ>À?)4€c«'?.¼œtLÂ?)4€c«'?î…Ç™žˆ?·š"ûý¼Ú?§£Øåx?·š"ûý¼Ú?ïÍ4®)ëÙ?.:©˜?ye¨ô¨ûa?.:©˜?ïõÛŸt?M2ôk¸?TIà¨ZªV?M2ôk¸AGN3FGL J0433.6+2905@eQŸÛÒúÀ)3UÿæՍÀ7胦MàÀ:ÑñËu?æ(Äwò3@Vmrõ@+&`;ÿà¿Øk®h¢p¿â-ôT"¿à+=ðÈÌÚ¿ßÎЇ\$AGNbll@$%ýŠÚºPowerLawMG2 J043337+2905?ïæ¨:Ç&E?«é:ÿuæ?iWÅQ–ë%?«é:ÿuæ?ï»ó×[`?'ÐÖ­ÝYž?9}¤?'ÐÖ­ÝYž?ï†X3ŒŽ?'•¶K†/<?Ž©èÎ'?'•¶K†/<?ïúАY]?,î»1ü¹'?G¼½Hgþ7?,î»1ü¹'?ïþ¼Ì#¯ˆ?$ŝ¬ù"–?$39{·®?$ŝ¬ù"–?î~‰m|…7?µ?D)È?¨i%£÷˜?µ?D)È?ï»B{"m?‰C!°y£?/a.¨×?‰C!°y£?ïïúÖS?RxR#œ½ê?`çmF¦?RxR#œ½êAGN3FGL J0433.7-6028@pí_ôöÀD'ï¤hÀ9*ÜÇÔÀ;É'o°'?ãód»|ª@æ'M@–?Çì¿Ý&â k¿æ$³­ZÛ]¿èØ7»x¿ïþÏë݀œAGNbcu@ýò f<uPowerLawPKS 0432-606?ïü•ø¿?>îÞÄKÇ??cO«bû?>îÞÄKÇ?ïÐ
(ÝnÛ?‹·aF:"Æ?wùkw+Šd?‹·aF:"Æ?ïWæYCpÌ?‹w¦i[šM?•4ÕÚŽ?‹w¦i[šM?ï÷§œ"?7@ÄQçEú?PáÂçÁ{Ó?7@ÄQçEú?ïûaŒPʍ?F·°H9z?ByÏÊ7, ?F·°H9z?ïDၘNž?ªü«so?—cÏË>^3?ªü«so?ï*¾''?•þvÐÝKÍ?œZ½†ußÝ?•þvÐÝKÍ?ïÞW¯ûl?cöl >?pÔ'⭖Ê?cöl >AGN3FGL J0434.0-5726@p¯ 6mÀDq™_·ö|À9óÁ¯bYÀ;ٔ¦ë'´¿ªù[?ÿç@'Ùv©T£?ÿú•ÀF+³¿ç;áVûi¿Èx½Òš'o¿äX"ƒv±¿Òé`VVúAGNbcu@ í'hr°PowerLawSUMSS J043344-572613?ïÿ3ÞLQ?õJmÁ?Ÿß¹@8‰?õJmÁ?ïÖl%ö'L?‹uVõá?tÉì÷¨V@?‹uVõá?ïÑ	×^?}½µ€ž¦?w{m%?{?}½µ€ž¦?ïûžhO8'?.•Ié?A†^³œL?.•Ié?ïþ‡œŽbü?'
v8A"…?'†4éY?'
v8A"…?ï#NŠìF?°™ÊPåƒz?›–.OÆ7?°™ÊPåƒz?ï̸÷-•?%B'ËA?y£"ˆ÷+?%B'ËA?ïÒcO¹.h?kµov¥	Ð?vÎXø?kµov¥	ÐAGN3FGL J0434.0-2010@k8
¿cíÀCx–@HÅlÀ9×
bY'lÀ;Å
ÎÜd?ðz8ËxŽÝ@m³Òê@–!@l³?ïù\œQôƒ¿Þ³4²‡¿æõb!£ò¿ê#£7AGNbll@'p‰ 'RPowerLawTXS 0431-203?ìZ‡'ó÷£?¿$Q1åš?½+Ãp`Bé?¿$Q1åš?îŒ1
9?«i\IˆÞV?§>ÌòÌ
¼?«i\IˆÞV?ëªëhK÷?®…ØώF?ÁW¼R^Ð#?®…ØώF?ëΜyE?šØÀ~"az?Àŏ‡®ì?šØÀ~"az?褏/Í?ÈoM€;y©?ϽmÃ@˼?ÈoM€;y©?鯎}ܤ±?đBêý ?ÉAƍm;?đBêý ?ßgSÎ>?ÁÄ·åžU?àLvÖvá?ÁÄ·åžU?àM…ƒPñ¤?¶ÿæ`¹×'?ßdôù^¸?¶ÿæ`¹×'MIXED3FGL J0434.4-2341@kć rѯÀCõöÿ¦=íÀ9ø*/~rÍÀ;Ш•µßJ?äèþ®òf@{'Õ‡ÜX@ÃÛËÍH¿à>+•ì¿èæÈtVÉ¿ãÿ©²&¿n¿ääµ
_AGNbcu@Vÿ˒:*PowerLawPMN J0434-2342?ïÿoÀhv?Cabh¿?õ3"1§?Cabh¿?ïÃÊ>Êb‡?~žH‹Ð|?~à}BÔ?~žH‹Ð|?ïÛÑåh?eäµô.•´?r
Q9?eäµô.•´?ï.\*3–l?sµH_F5?š4z¹2Œ?sµH_F5?ïþ/×ø¾²?2^µÙ?-*™¹?2^µÙ?íÓaZ§°"?³·´¢3œ?±dõ)x¤u?³·´¢3œ?ïCQ[gYÖ?'I×®_öÌ?—•Ô"Ì"2?'I×®_öÌ?é™è5!ä›?¨Á&*?ɘ_+xm"?¨Á&*AGN3FGL J0434.6+0921@g^­@ªêûÀ8Ë@—ŸÄÀ9Í
eÀNÀ;‰pà<ìÀQ4MdŒÇ@&`ú–´@êè CZ¿ç™ØÕTìӿُW¿Ûu#¨¦§Ê¿èÔ;D_ç'AGNbcu@ M:'£PowerLawTXS 0431+092?ïú¯ÿ¾?ESÆó7NZ?ECç·~?ESÆó7NZ?ïÎ}TУ?ŽZSB#9a?xÁU¸ª¿#?ŽZSB#9a?ïÕæ4Ž
[?u'u#r¿É?uå©Û
É?u'u#r¿É?ïÿô"bf¹>ÓRP¤OB>×»,'–I>ÓRP¤OB?ïò#·!â?a•ÐøÝ¢4?[¹À'¼;Á?a•ÐøÝ¢4?ïQà#…"þ?¤vãiÏÚý?•Ãû'¾ü-?¤vãiÏÚý?ïyïdý/Á?'Có¨af*?Âg9?Õ?'Có¨af*?ïþòxFÒf?"öÇÚÂß? Ø{
'·}?"öÇÚÂßAGN3FGL J0437.2-4713@o«˜€"åÖÀDüsßË­À8¿qw; ÀÀ;Àîû.	@šõº+àY@	«¼üK@ø/M˜w¿Ò´JÀ²¤¿är>Y_ W¿ë·D)Јï¿íĬ妸fPSRPSR@'ˆdâmHPLExpCutoffPSR J0437-4715?rã‰nR"à?®>mNè?ïÚ8íK6N?®>mNè?º¨²2ºò?ÊC"¡"c?ìªé¹¨¾â?ÊC"¡"c?Ãî"²Ýb?­ ¥säÌ?ë9DwSH§?­ ¥säÌ?V!vÚWæ?C¨€ïT
U?ïôïDŠ¸D?C¨€ïT
U?qÝV®÷†?zÚœÈ%?ïÜERf÷}?zÚœÈ%?¬­X©"'f?ÀéAå y?î5*u/¾?ÀéAå y?·-j}ׄ&?¦é窸j?íR°7Q?¦é窸j?Ӛ¢ØŖ?
[XÊ+t?ïÿic=S?
[XÊ+tPSR3FGL J0438.3-1258@j;4 -œñÀAª(CìÀ:/rq6¤À;ÀlÄNy¿Ó'èxWˆ0@ú¥>hp'@Ù f|â¿ÞAš»>¿çÒúdúDn¿°pN$XØg¿ëV°j¸ÒçAGNfsrq@¡؆YJõPowerLawPKS 0436-129?ïýƀò¬?(š¿K_"?1Ë÷îv?(š¿K_"?ïɔÌ3¨?'Û汈Y?{5÷'§à?'Û汈Y?ïsÝüŽË?‹œÄhnj?'DCÝ—?‹œÄhnj?ïø€ÉÄ?9‰1«ÿÒ?MÊ3?9‰1«ÿÒ?ïýÊNü?=ÒÁ6S?7	¬'4?=ÒÁ6S?ï$ä@åV?±ýߥÆ&?›cwè|¨3?±ýߥÆ&?ïYŒ¥âŸ"?"X‰IŽk?"ÎkLCj?"X‰IŽk?ïÑXš Õ£?rÉŸ[þ?wS²²TÞw?rÉŸ[þAGN3FGL J0438.8-4519@oY._ú;›ÀDåù jn3À9?ÖbwÄ]À;¾s"LS?ëÅ`ûK@^d‡éîÇ@!¥?êüŽ¿â¿®{¿äpqÎ_°%¿è
žªÁ¿æÀVò!'nAGNbll@ˆBàÞÓPowerLawPKS 0437-454?ïßgՖ?pË7ݎ$?pvLƒÍ?pË7ݎ$?ïPËè~â'?"Ÿd<s+?•æ'êüCÐ?"Ÿd<s+?ïh¡ÉKõ?ŠÜdrÚãÈ?'ëÝcfåd?ŠÜdrÚãÈ?í2X)·´b?™QœÁˆ?¶m>±Ôir?™QœÁˆ?ïÒJý)?ŸÉÖD½?œe¾ý'Ê?ŸÉÖD½?è{¯'™?ÊÙC0ê%?ϾAµ›È?ÊÙC0ê%?ì}t¤0/?©SëæG¼?¼ZÞ{~"?©SëæG¼?ÞÉÎäØÀ?¶ÛÔ1pˆ?à›ü" ?¶ÛÔ1pˆMIXED3FGL J0439.6-3159@m"†_•'ÍÀDZ{Q^—À:fùû@ýÀ;ÆõPy•¿ùh80)1@ÅB' Ôa?üT}?ñ²Š¿ïý¨é²z€?ïýÎ'üÚm¿éDúöÄå?ÆÁOòlÕ§AGNbcu@³oŸ¾wPowerLaw1RXS J043931.4-320045?ïüœ(¶'?<ïG{#–?;º"™áÍ?<ïG{#–?ïÐôœ?È/´AžX?w…±Û†ÛE?È/´AžX?ï¢&Ñ%!"?zz©¶?‡vK¨ùG¥?zz©¶?ïÿõLâuš>ÓÀïCöxÿ>Õeäj;«È>ÓÀïCöxÿ?ïö÷%ù?Rb¶uܽ?RäÇN>?Rb¶uܽ?ï8ì‰ðH?²nr˜?(?˜ânÇg=?²nr˜?(?ï;ÒîÇ?ç?Š94ï?˜…¢(ÏÑ?Š94ï?ïþ²×œù9?+éâ¯6D_?$Ҋh$×ö?+éâ¯6D_AGN3FGL J0439.9-1859@k(¿;ê'ÀB $€	À9Õ~ŽÑ¿À;ª7Pþ¿õ'óžá@f' 'ìÚ?þµá)¦¿çÀØˑA¿á>š'LËá¿Ú¨—Êr»›¿Ý¸7´¢3œAGNbcu@¦SZ…‡"PowerLawPMN J0439-1900?ïÿ'2¹'?鈟N&?sIÝõ…?鈟N&?ïÓzÖµÙÁ?Š×'¥mý?vB"ێ?Š×'¥mý?ïìySÛ?o-ö0»?cæ†Oñu?o-ö0»?ïÿêÝüS>ßjÄ#2³>åï3RÞ>ßjÄ#2³?ïÿgÝÅÿ?
´7ˆ›)²?IÇõõ?
´7ˆ›)²?ï=h®j6*?±"Wèõ!€?˜Rê2¹:Ê?±"Wèõ!€?ïð˜~?gL‰0ðק?^Ï]Ó\î?gL‰0ðק?ïþÛø0JB? 綌òè?"@~ß$Üb? 綌òèAGN3FGL J0440.3-2500@lT2TçÀCÿ·äÀ:ԕ(ñÑÀ;í(åÒWP?êìãZON>@yAôl#?û–×6&-¿ïþ~ôãÓ`?ïþÒúb¿²@gÏ2f¿éölš:²AGNbll@³óVÈ´9XPowerLawRBS 0570?ì*˜ñí²d?ÈFì)ºø?¾«8p'lÝ?ÈFì)ºø?î5Íæ8"Ø?²
ƱÄwƒ?¬£!Ÿ
gz?²
ƱÄwƒ?톱¿Ï?¤ˆÉyÇqb?³Êr7	Š?¤ˆÉyÇqb?ì}õ³ƒG?£ûÈfJ\§?¼WjcåÇ?£ûÈfJ\§?í¬aþ³á?¹UÇùGb?²ŸŒïœmz?¹UÇùGb?èÉýVYg?ÊõV_Cm¤?ÌØ
§'šf?ÊõV_Cm¤?êŸ¦'?¶¹Ä†C?Ḉeù·š?¶¹Ä†C?潌p™Ï?ÃÎñ·4W?ÓЄçÌc?ÃÎñ·4WAGN3FGL J0440.3+1444@fåw'þLÀ4zƒ?»òÀ9WIáËa"À;Ip:$¾ü?â
!÷N@]E€gÄ@(k 7™¿àh•ž?ú¿æn¦ü®'οèºçC_j
¿á ¢Ç둉AGNbcu@Š-Ù_í¦aPowerLawTXS 0437+145?ïçf¨Dq
?yF€Ú;cn?h™W«Ó ?yF€Ú;cn?ïŸÐ4š?ŒŠ¯äC*?ˆ?Œ1Iv?ŒŠ¯äC*?ïbœ#P€æ?‡XCýŸ—N?"¬{•ïãJ?‡XCýŸ—N?îï§Ñr	?€97QK‡H?¡'ìql?€97QK‡H?ívdW1Y?¹o]Â|1—?´LÝGQí?¹o]Â|1—?ë_¾´lÈ?ÂÚÅÅãk?Á.LÞ?ÂÚÅÅãk?êË­Ëú?µ«•K{?ÄÒKüÐ?µ«•K{?åì(3i¨ª?¶5'檖?Ô'¯™,®¬?¶5'檖AGN3FGL J0440.8+2751@e'@¿ã°À(h> Ìÿ"À9È£¥¦îÀ;oW6Gºª¿Í
à6i§@2ƒÄ›%
?ÿ0/}HÖ¿Þ^ëì*h½¿é
M`äyð¿Å³Ï¿Š2ã¿á±¾™XV-AGNbll@°Ü¡aä÷PowerLawB2 0437+27B?ïÿng37\?U¸W7?3Ž/• ?U¸W7?ï¿ßž-"?ïíyš¿—?€~¯9?ïíyš¿—?ïìÖ0^þ¤?\‰®ôƒwÕ?c)Ïy%ãñ?\‰®ôƒwÕ?ïûä2?'Ô'û5ÿÛ?@oô	ú¯?'Ô'û5ÿÛ?ïþš*îÛ?+9Õè±sˆ?&^φ8uÏ?+9Õè±sˆ?î¿Êñ³ê†?©Å0½‹\?¤Pâ-¢Ÿ?©Å0½‹\?ïå$f´'?nÙò*Ñy(?jۙ`'%­?nÙò*Ñy(?ï挎T}?_hF:þT?i€sWŽzã?_hF:þTAGN3FGL J0442.6-0017@h¦€Ÿb0wÀ<vŽ ¿"(À7±åvø…À;EŒ^G³ô?çÒ4oý@»O)@÷Íÿ§Ày¿äê/ô^'¿çÜ+0ý›¿æÃÔ;è¿ë›‹¤•¡AGNfsrq@{òɚé$òPowerLawPKS 0440-00?ïþ¢Þç¬?%…+{a¡?.…Ðfèî?%…+{a¡?ïÊÅü׊?Öuæß?z[¹2?Öuæß?ï̲ÿ#ë?•'!"ë®?œÆižc´¯?•'!"ë®?ïþíášdE?
ÎÇ Ò!*?!!ä¬ìur?
ÎÇ Ò!*?ïýƒe
4?3Yyë5G?3äÔ«3²D?3Yyë5G?ï9]7yÐ?¬'­¼2Ã?˜ÔYíh~?¬'­¼2Ã?ïNÏÔ>0<?'çœzØ5?–&v'*w?'çœzØ5?ïýæ#¤¹¢?*R4Æ@½?0Îä]: Ž?*R4Æ@½AGN3FGL J0444.5+3425@dþÊ€àÀyU E…EÀ9æoD[y£À;O®²0?à3-;Cð<@¦|«ø@wÈ_ÂX¿ Ôrªä¼û¿áýò?¼È¿åQeà7@¿ê½ZÅÑäAGNbcu@¢.Xâe,PowerLawB2 0441+34?ï'=‹ëtò?'"ŠL[?‹°q—Z?'"ŠL[?ï'³?'äRrt¯?‹{:ñ´?'äRrt¯?탄ÿP$'?£ÞOä?³ãØȹE?£ÞOä?ïj±í«ó?l£° ª&¨?'©ÂGB?l£° ª&¨?ìÚ³Mu?¹HÁ!äOw?¹/ɹÛ?¹HÁ!äOw?ìÇ$å½?¾ñ4?¹ÆØ×rJ?¾ñ4?éE:C•"‰?³R8=%}Ó?Êëñ«uÜ?³R8=%}Ó?ë§FÖS3Y?¡ø$òÜ3¦?Áb䦳2?¡ø$òÜ3¦AGN3FGL J0444.6-6012@pàŒ€AÀCs`ûH
À:\f('ðÀ;ïë‹Ô´ù¿òaohی@^©WQËz?ÿ™¾×ü¿î#ߜ]?Áh%£8æ¿à•€œêÔA¿Ö7‹~ñ*AGNfsrq@¥ˆ6E¡ÊÁPowerLawPMN J0444-6014?ïÿI¿Å/þ?™¬žCÕq?ÈöšéÛ?™¬žCÕq?ïڝ
où?"˜¶'¤Ö?r±zÌ"ýŒ?"˜¶'¤Ö?ïçYÍ?¨%?aLJ~!ò°?h¦2ÎJ†?aLJ~!ò°?ïÿ±Fg (>û‹Š×ÑI?®YËK.>û‹Š×ÑI?ïÿðßÀ?ñˆ¯ðªÄ?ÿÅy¼­?ñˆ¯ðªÄ?ï.>öF)?²ŽìMÕÖ?š8!>K?²ŽìMÕÖ?ïÞY)g—?r)@?pÓkkk°i?r)@?ïû;:ØÄ?>¥o"‡Âi?Cƒ½cXÀ?>¥o"‡ÂiAGN3FGL J0447.8-2119@kŽ± ‹ü"ÀB!ÕߛªÀ:Q˜y*À;ÉlËu±?ÄhÔÏ>…æ@GrÄm­­@`¡ ¤$ã¿äY@í ¿ç֗4u¹§¿åÍ‹gb÷¿ïÿ{j£ýAGNfsrq@…ßoÒóPowerLawPKS 0446-212?ïüÀjS†?95ü­Çl?9ÿfÕ¿r?95ü­Çl?ïŜJŠ#?…ìUN4í?}1Ú§°¥{?…ìUN4í?ïe•gt%?{'UÔZ?"MSDñq?{'UÔZ?ïCäO#8?xF¼rL¦´?—ƒv<a?xF¼rL¦´?ïü‡Í¿;?>Éښk´Š?;Á"¹x«?>Éښk´Š?í±ú¹ø'V?¶¦´CWÝP?²p*/_†Q?¶¦´CWÝP?ï%C…T¬ï?'ýfя7?›WS²"?'ýfя7?ç՞£LSs?³âÆ=¤l?ÐT¹gY?³âÆ=¤lAGN3FGL J0448.6-1632@jà»ÿŠ;ÀA6¿Ý/ñÀ9AÞíwÀ;\ä
[2V¿àÉ`í¼Â¥@'_?ý¶¤^ïy ¿ÅÜpGª¿Ýˆ_ãý4¿Õ»Ö[åÚ¿àXU¨9UÈAGNbll@¥Žèۋ¬qPowerLawRBS 0589?ïýÃ?A?1Âq^‹þ?77âGáA?1Âq^‹þ?ïÓ[²¶Ôœ?‰ŸjˆÓZ?vR&¬ÔÂ4?‰ŸjˆÓZ?ïÕl3~·?p`æb0´ñ?uIæYŒøo?p`æb0´ñ?ïýؚ$GÍ?!ÊÿQR?1;/_¦`?!ÊÿQR?ïû"k·?<ÉAù%?A¯…Ì¥Þ5?<ÉAù%?ïA¦üß(?°ÏP‡:@?—Ë< dÿ?°ÏP‡:@?ïÃЋH?PV}e?~ºSœãè?PV}e?ïï}ôf?U²iZÊÄ?`'+©v?U²iZÊÄAGN3FGL J0449.0+1121@gm ìt2À4ª_ºz»À7䨮àR¼À;:ŠE–ã?ý€qÅ?9Ò@¾‡d¸¼@¼³Ž7eÈ¿âFWÔ8 ¿éU;)]Ê¿è[•'ïx–¿êÙèögêAGNfsrq@rj¯·éùLogParabolaPKS 0446+11?ïìFfZ–¾?uóÂ
Ì?c¹™r
?uóÂ
Ì?ï*A$Á&?°¶íÀ| ?š·Û`ÿÃF?°¶íÀ| ?íP(y?§XÃpşc?µ~»'íÌÚ?§XÃpşc?î@'ÀìÍ?Ž?5õÛ8ö?®ý‡`Ï&?Ž?5õÛ8ö?ﮑÉt0\?Š;bÞoØ?"[¢›òú?Š;bÞoØ?ì´âT0Ú?Á4Þë£?ºXï…^y2?Á4Þë£?íäÆ	t¡?¢"]˜¤‹—?°ÙϵLŒý?¢"]˜¤‹—?ëDµZP"©?¯Ã0P[¶U?Âí*–½­[?¯Ã0P[¶UAGN3FGL J0449.4-4350@oΠwmÀCôäàõÀ6Ñd‰"—À:Léki¦?åÅ~Ä¢@Á]Z¤k?ý•\ ¿Ó•¿ÜFž†#¬>¿Ýs䧯޿؉k?$iR¿Ü+ƒÆAGNbll@"k]æšÔ,PowerLawPKS 0447-439?ïã»Ùµh'?zF=sÍ?lD&3:&?zF=sÍ?ïÖ^+.ô?‡\áÈSä?tÐêjÎÊ8?‡\áÈSä?îyØûü‡?¡¾k¡hå?¨bpAïT/?¡¾k¡hå?ïúbÁ/#ž?4c,}3@?Ftü r?4c,}3@?ïæÉèì¾?pzÆÉQB?i6Ø(´v?pzÆÉQB?ï\6a»Ý?´38î·?œy<_Š]?´38î·?î¿J[v{æ?¡Uã=OâY?¤ZLãĜ?¡Uã=OâY?ïóMþCE?P1
Ú£-Š?YdMzü²?P1
Ú£-ŠAGN3FGL J0453.2-2808@l¡i@5z5ÀB'HàC¢À8iüybÂmÀ;ŸüJhÙÞ?ôPBàÐ9ê@ÓÇ©¢PL@
€€mùƒ¿å`tԊ¨²¿èýhæÉM;¿éf¢®7­¹¿ìá£ÙŽ|/AGNfsrq@xB÷zö@dPowerLawPKS 0451-28?ïë¤xð­?lX‡J ƒâ?dô[®êË#?lX‡J ƒâ?ï½Ü­H*Å?ˆ«iì&-?€ˆÔ ŽÔç?ˆ«iì&-?ï¡V¸0?W¿"Ú?‹ÕCcë?W¿"Ú?ï&š›Cµ.?|Ämª>?›,¬ª"L?|Ämª>?ïñÇæ^d?c<ªÂ?6î?\p3´'g?c<ªÂ?6î?î´ˆQƒç?°E¡bò±?¤¿ç}{v†?°E¡bò±?ï2aه?"Ò?Ft«?œ™³á<?"Ò?Ft«?ìv=½‹øW?¨;p{¾?¼N =D?¨;p{¾AGN3FGL J0453.2+6321@bNO€Ü3r@(Y?µ!µÀ9v(ßóÀ;[‡æï?âEi™KÀô@'–E&@Æj?Žá/¿ç¨8_å:N¿ç⪬]ãØ¿Þ²~UNÅ¿ÛÀŠ0'flAGNbcu@'ñ[W>«6PowerLawNVSS J045312+632117?ïþŒ%Î×Ð?><"¶J¹¾?'=¤È©?><"¶J¹¾?ï½Î2}g?*Ëîq}?€Œz¯™I?*Ëîq}?ïíÜ
œ*?c‹5ãǧ'?b#õKÉ¥?c‹5ãǧ'?ïކ\"Å8?P],¨6,?p¼Ñ¿ì7Î?P],¨6,?ïþ5†¾?0q¢à?.l¥"^}?0q¢à?îpCö隨?·uèzjcÓ?¨ûÀ"#ƒ?·uèzjcÓ?ï¼,N°×?QÕ%
a?€ôì|C¶!?QÕ%
a?ï9Teïj?"íÙÃÈo°?˜Õs<ø(Ò?"íÙÃÈo°AGN3FGL J0454.6-6825@qzw@=ݱÀAÚÁÀ)P[À9óLŸÀ;ª>"E]?욆 \p2@ðÑ›¯ô@"ä %\¿ãƒ"^ϙ¿äJRŸ	E#¿âB;¿┿ïÿ¸èz0OTHERpwn@›Às3333PowerLawPWN G279.8-35.8?ï˜öö/á?£þGð¹Îß?œláZËÞ?£þGð¹Îß?éäь‹O?ÃÛN¡3ýð?˘l¹ÍÒÂ?ÃÛN¡3ýð?ì"(eÇ&'?¥¦ù·{?»f¼ÑÆËp?¥¦ù·{?ælhš·ëƒ?§bü3¸?Ó'.ʐ(ú?§bü3¸?î@"µÂ?µ&åZ¯ø?«ÿ½ÓÊ<Ü?µ&åZ¯ø?Òﬧ#¬?Ð8uùg›¬?æˆ)¬n)÷?Ð8uùg›¬?ä·£zˆ?½5Ç£©?֐¹àð?½5Ç£©?ÆFÄ'5?­ûÝSY?ênNú[rº?­ûÝSYMIXED3FGL J0455.7-4617@o¼@ŽÉÀCi·?œÎÀ8Ÿ>õÀ;¡1$e:?ï.9Ķ˜@ßqBn=@^àAHË¿å^WµYÏ»¿èBs'‹ò׿çw'&Ç¿é¢AcÖßAGNfsrq@|?€If{PowerLawPKS 0454-46?ïþ]"
q5?$ÑV2J?*&À?$ÑV2J?ﵟ¡ÆcÒ?Ž¿VÐBä[?'˜'`iŽ?Ž¿VÐBä[?ïÇȶ4&p?o7Ÿí†VÍ?|¤ìÌ%?o7Ÿí†VÍ?ï,Õoø±?{þ4A.Ø?šeR±÷?{þ4A.Ø?ïü¡Þ¿?;yüÜ%ž?:óg¡PÜ?;yüÜ%ž?î)jùYXó?·
»ñ¸?­iPgÖ»Ô?·
»ñ¸?ï¨OD`Ø?…FÑQ•»?…ì.àêÆE?…FÑQ•»?ëY&^L?«íå«}ã?›eÃö†Ò?«íå«}ãAGN3FGL J0456.3+2702@eì&?šIÃÀ$ÔHµ{À8෋òçêÀ;-hÁŠyk?ñYžqŕ @Q¸Ð¢@®i t)¿àʵ4D¿èAÐ…h¿åP‹¿¼C¿ì8ÒXõ1AGNbcu@ƒ½>§°´PowerLawMG2 J045613+2702?ï÷¼P9¦?L†·Œ¬h?P‡_qy?L†·Œ¬h?ïB•nð+T? '¾éæç?—­R!ú•w? '¾éæç?ï%¯¾Þ"?ûLéœú?›J*ԑ~?ûLéœú?î$b*A?~âÔ¡±ƒÚ?­¹Ý^yäÇ?~âÔ¡±ƒÚ?ïî mâöI?dÉä²i»?a_'ØQ‡©?dÉä²i»?é~ÜJTs0?ÄÔҗ^xS?ÊŽÖ®3@?ÄÔҗ^xS?íÅùzïy9?£{5^êBÀ?±Ð4*©÷¶?£{5^êBÀ?ç´no|î?©Lý‰®%?З#!#Ê?©Lý‰®%AGN3FGL J0456.3-3131@m+VŸIÀB½¿é{À9ΈJ¼½À;æHEéï?áX쒇N
@㹯c°T@MbÀi'¿ã
ºægÊâ¿ç©¿ê;Gª¿è1Nˆ	Š¿ïÿãï—ìµAGNfsrq@Ú=!ÿ.IPowerLawPMN J0456-3135?ïÿ‰»*8
?ɬŠ?
')•"{ß?ɬŠ?ï¼DüB?"sЀ?€îýÈãQ?"sЀ?ï¸
á§È?l1LÝO?û½;l'?l1LÝO?ïj!¡¡Œ?oIÇì⚫?'½ÛËËÎ~?oIÇì⚫?ïÿ¤ÏÇlÕ?®q×â?ÌôÑDž?®q×â?î{Ôë1ðF?²n-"°nì?¨B±L¦?²n-"°nì?ï³üiG—C?'GÙÕi??ƒå²é£%?'GÙÕi??ë0>X»i?¤OWØõ-?Ã?î[?¤OWØõ-AGN3FGL J0457.0-2324@kö©Ÿ¡—ÀAr–¿Ê…ËÀ6uQ'ÑÀ:£º¤¬S@–íw'2È@ Ïryð@à"@¿7ä¿ÞÎmЁҿäQÍ_™Ã‹¿å–À™¿éxŽûAGNFSRQ@vÍ¢±pPLogParabolaPKS 0454-234?ïñ¢Âi?X	UÜú'?]Ê»¬¿=O?X	UÜú'?ïДrhRO?ŒìÆéé%9?wµÆãäs?ŒìÆéé%9?é³ðš²Hg?±Äjþé?É0=•6Þc?±Äjþé?ïþÇIäY?ò}™É?#‹l¿×‡Í?ò}™É?ïc/9Ôb?ÞŽ~ˆq?"šÇ+‹?ÞŽ~ˆq?ï6ì3M
?®"¿â{J?™"y"¥ð¾?®"¿â{J?ë–ãuŸƒ?®»Ô¥~í?Ãͤr)ó?®»Ô¥~í?ïÿ‡)€>?ûOÏ&¼î?5òDo'?ûOÏ&¼îAGN3FGL J0457.0+0643@hDàÚ ËÀ5°cÀ™¸£À9ämBùyÔÀ;r#QA;¿ÿzr·Ø@ÎÆQ@a:ÿZh¬¿é ?Ðû[¿ãu&ǃÑu¿ìù×bä¿¶õÅÿÔ0AGNfsrq@Š©0 ě¦PowerLaw4C +06.21?ïüôze̸?AÓÁ€¹Þé?8\.ÞÌ\?AÓÁ€¹Þé?ïÕ~"•PŠ?…2–yU`Â?u@½JwI?…2–yU`Â?ï¬1Til^?}så›ËÜ?"óªÛV™?}så›ËÜ?ïÿþVBèï>¨Ž7H<P>ªšéf•'>¨Ž7H<P?ïíT•"¸p?q+þ{e?b«j.ÎpÐ?q+þ{e?ïàßiÕ?²ú|/éÑ?œÃÿ	:/_?²ú|/éÑ?ï#7Nd«À?"â+h?'Â?›™,‹P
?"â+h?'Â?ïÿÀéz-?µ"Y«Xu>ÿð€= S8?µ"Y«XuAGN3FGL J0500.3+5237@ctÙ_í¦a@e©ÿî7VÀ9h ƒ-FŠÀ;]€
|ZÄ¿Ó`…'F§ë@
[¿Pã@Ë àJX¿âæ=@¿ëD8>4îõ¿Ýa'Èýµ¿Ø—ÁREG2OTHERspp@"?ÂIº^PowerLaw?ïûoR{Ö?Nãž'«(?CÒAäíÓ?Nãž'«(?ïÂz·½WJ?ûN)(¤V?~¤†'?ûN)(¤V?ï¯ÖýèE?~ž›;þ.?"
~'•²¶?~ž›;þ.?ïöñœ÷g?<ò§y~C?RÅÍC$?<ò§y~C?ïçXFñ‰£?rƒRæBóÒ?h§¹×tØ?rƒRæBóÒ?î¬u'G?²±žðfG?¥8®0D£?²±žðfG?î²Á ßV?œv;Q¬ôT?¤Óç$:<ª?œv;Q¬ôT?ï‹í­~9'?…Öàù1á?"£áR2?…Öàù1áAGN3FGL J0501.2-0157@i.
á'6À9E  œWºÀ81dÒèoÁÀ;Zl ºŠ«?óÿ2ªøÈ@³¬wâÆ@OB?ë}g¿ã÷|k¿ä¿æ@àùˆ¿å¥\jÓ¿éñ•S0KAGNfsrq@•Â&€PowerLawS3 0458-02?ïú5(€Ó?CBñø'«?Gã+›'ë?CBñø'«?ïÄNL¥[?"Â×(|*?}öX·Q:…?"Â×(|*?ï§k€ùÜó?«»Ö=w?†%ÁˆÃU?«»Ö=w?ïòUö?A°çqUù²?[ñUŠƒÐ?A°çqUù²?ïò+?2ü?X2P0+XT?[©ò¨?X2P0+XT?ï,ÔÿSæ?­Ô]FÏi­?š…c…4?­Ô]FÏi­?ïd?>љ]?'Kýô%ðï?"x ¥jr?'Kýô%ðï?ïâràa
?a™ÇBÈr7?mÈ#C?a™ÇBÈr7AGN3FGL J0501.8+3046@e¤(?NÊhÀ5pÿÇuöÀ9Íøí½]À;WQ§'€¡¿ÈW%«¶&Ã@ÃɃl0«@þÿÝp^¿Öfm†¯ö¿éíq—
â̿췋aiô³?æÉǓkÆçAGNbcu@§ËàÞ҉PowerLaw1RXS J050140.8+304831?ïú¹–Sô?WñF…ž°?E§: â?WñF…ž°?ï¶Õ´Ij¥?"ÅE-¬l¢?'J'Þ/ô?"ÅE-¬l¢?ïH	E<äÒ?AõÛÉEØ?–þ×V«—Ð?AõÛÉEØ?ïÿÕ69F>ô
P˜œý>õdÿœX'V>ô
P˜œý?ï×HV¹}Ã?xÃu
óí?t[ÔªÐB_?xÃu
óí?îk­xÈé?·rö|$'?©E(}GŠu?·rö|$'?î N^Ý°ö?¡ƒ'`8»?­ûpsŸ?¡ƒ'`8»?ïû°U{e/?MqÖ5gGZ?A>©üú'?MqÖ5gGZAGN3FGL J0502.5+0612@h>ìß&k¥À4Ó>¿XpÀ9ƒÂl º‹À;'ÅPÉ?¬î"É€[@µž´5§,@¥¹ß_K•¿áS¯¸пì4k‹>b¿áÁÄ|àë¿ïúÕ	öè™AGNfsrq@‡yFsØPowerLawPKS 0459+060?ïå3UÂÕ'?mS 2)?j̪OЮ?mS 2)?~_bLb?'Š/†då[?€˜h ¯¥?'Š/†då[?îg¡åBr?šYnÉEá?©…á«×æ?šYnÉEá?ïžKîH¦?oígù@Ð?ˆmc‡¦â?oígù@Ð?ïŽþñ•·•?–"˜}3ä?Œ@C«À&?–"˜}3ä?íþ~T–Z?¶ÇNYÓ{«?°lf/?¶ÇNYÓ{«?ì˯ÿ¹G?ªÉ#ÔSPu?¹¢€¢5Ê?ªÉ#ÔSPu?ì_èçú>?¦èüÈùê?½¸À.Š?¦èüÈùêAGN3FGL J0502.7+3438@eD¼@ŽÉÀ:ƒ?»òÀ93u@ô¼ÖÀ;=KË°m?ìN–ž×@èÆUå9Ö@JL`€É>¿áÿVÛ6¥Œ¿àKTš¿'¿è:¼¢ï>ù¿äû¹*>ÔAGNbcu@'—ÊÚ¹õZPowerLawMG2 J050234+3436?ïý%3ù?:ÿ6pâR?6×çt®?:ÿ6pâR?ï |¿:µU?"OôθN)?‡àÐ'ÖÍ?"OôθN)?ïŒ3ÒÀVÈ?"ìBmi¹"?ŒóE›z ?"ìBmi¹"?ïÞqÌd"?M6‰8'U±?pÇà ò?M6‰8'U±?ïéìÙæ?i¤›\'ª?fûêR^é?i¤›\'ª?í} aÊJg?¾uìãÿ3?´üò÷‡J?¾uìãÿ3?îj9®™Ó?›ÝN.ŸS?©V,d:{Í?›ÝN.ŸS?ï^}^z‰´?'`ÓdÕ?"0T.öû"?'`ÓdÕAGN3FGL J0503.4+4522@d7  ôØ@¯rú6<À98‹ò)ôÀ;3>iȶ?jÐì1»@˹ÕÁ@á€.¹|¿ÚÁFíá¿íqÑcµ\¿¹õ¯ÞÄ4è¿áO.+AGNbcu@'¡h	ԕPowerLaw1RXS J050339.8+451715?ïþÚÀDB?%÷º`rÙ?"Sýf{'?%÷º`rÙ?ï¿(DÛ9?‰ye«?€5îú¡'Í?‰ye«?ïÞëL>È?rࢢõí?pýŠ?¨2?rࢢõí?ïú骠tw?0SS{½Ap?DYV]a'<?0SS{½Ap?ïþ…›'t?(y2É'Øy?'®7ïY6w?(y2É'Øy?î,ß¹…êˆ?½³†æʶ?­2fÅpˆ?½³†æʶ?ï.Zö	¡?Š \
a?Œ´i1O‹â?Š \
a?ïìdÕA»?W¾?[¦I?cbšçeìü?W¾?[¦IAGN3FGL J0503.5+6538@b'Î ‰ãC@,Ñeaƒ¨—À:X4õ«hÀ;ÇPܑeî?Äà5Á¿å@.ûJ¹@®h@0FÅ¿éqÏÔÐ7¢¿Úü›Ö׿ì[
'ÁË?Ù£@'ªAGNbll@¢P1Þi­CPowerLaw1E 0458.1+6530?ïú9ku]¿?V,þӆ+?GRÙ1[?V,þӆ+?ïÍXÇÜü?‰y`—"|?ySœÎ?‰y`—"|?ï|u$!ü?ƒ€).Å3Õ?‹àâ©9?ƒ€).Å3Õ?ïýÃdX?*¸YÅÆ?3ñåDdïs?*¸YÅÆ?ïÁu
šÊ?'i	Ñ1'Ñ?E{?ÞÕ?'i	Ñ1'Ñ?îÅþ•$r"?¶‰0!e=b?£ ­¸×Å?¶‰0!e=b?îi¸2‹î`?¡mÌt'é*?©d|Ú°µ÷?¡mÌt'é*?ïNjjŠk?€za™Bɹ?|:JÀIÜð?€za™BɹAGN3FGL J0505.3+0459@ho0_®¼AÀ4ÜW?öÀ86ÈqyŽÀ:ô÷eýŠÛ?ûaܶ#é@ób–x'@Ïï=*¿á½Ë"Ú¿æ@*†!¨Ø¿éT‰;Ÿá¿è?nO"æýAGNfsrq@1äÂø7µLogParabolaPKS 0502+049?ï÷öÜR@?]ÛòÙ'?PG†STç?]ÛòÙ'?ïÁSöˆn4?ŒÆ×t®n6?VÛeM®?ŒÆ×t®n6?ïJòP%B–?'¤6ÇâÂ?–¡µþÇI??'¤6ÇâÂ?ïð±']V·?F›Ó©<Y?^œû¶ÁN?F›Ó©<Y?ïêâž4!ß?plë•)½R?eaðùèe?plë•)½R?îô¾äŠaK?°×cjè¿? ´¸5ÒO?°×cjè¿?ïÛш¯x?–AnÂý×a?œ$…ÒY­?–AnÂý×a?ïèPƒY?aH}Vɹ"?gþñy⿇?aH}Vɹ"AGN3FGL J0505.3-0422@iŠsÿ¬*À9…Üßi‡ƒÀ9Лx–ê"À;pæDm[?ó[
/')@
֕Î]ñx@
ú`-è¿ÚeÙµàÄs¿ä˾mA*¿çÏé°Äi¸¿ê™¸õˆAGNfsrq@•¢aG®{PowerLawS3 0503-04?䭏ÙK?Í>…TpÎ?Ö¤àM÷Éj?Í>…TpÎ?âÑ./àÅ?Ì]ñUuÛØ?Ú]£ >àw?Ì]ñUuÛØ?êµ&M¥,þ?­$3 rO?Å+fÉkL?­$3 rO?äLV×kûë?§ðO)?×gRQ()?§ðO)?Äp|"ÿù?ÄoëU#?êãà÷@½?ÄoëU#?ÄÓk=vê(?ȏÉÁÕwì?êË%0¢Ev?ȏÉÁÕwì?ÔńæÑ}-?»±y4I]Â?å=Œ—Ai?»±y4I]Â?Â#Âû›Iû?£ÀÙx§'ž?ëwA-?£ÀÙx§'žMIXED3FGL J0505.5+0416@h…Ÿj"óÀ54"Ÿ^ÕxÀ9Џº–iÀ;vVO—íÈ?ÒG»_ç5@<OM:?þ}q +Y?ÝÕ«:"]¿Ñõ¿èÁS¿¦FöLпäHMÌ#1AGNbll@±®lÌÌÌÍPowerLawMG1 J050533+0415?ïûþ#K?aLzz³8?Cë³›²ñ?aLzz³8?ïÆ.Qeè?<ô©gôW?|è×S;Ké?<ô©gôW?ïÓ ZËJ
?o"|ðw<?v/Ҟz_?o"|ðw<?ï˜UG–RÎ?q?2¢•?‰ê®xt?q?2¢•?ïߜWäîW?zIœ+ô=h?p1Ô$6@†?zIœ+ô=h?îp@Zk¹ë?±¼'@¦R)?¨ûúUÔÅU?±¼'@¦R)?ï¦[MGuN?†ŸÜ IC?†i, d<?†ŸÜ IC?î_¦Ø‹5Â?™Ä]žˆð?ª'sÝÞ?™Ä]žˆðAGN3FGL J0505.5-1558@k&€IRÀ>uàè@À:7œÓ	ý°À;͵±þm¿àšŽX•9Û@
2"¤Åœ­@ÐúÀP»¿×'ƒk7¿ábvs5¿ç •—‰ýx¿Ð[±e¬ñÕAGNbcu@Ÿõ}<64PowerLawTXS 0503-160?ïýX»'øm?6õ"0c»Š?5:&e8P?6õ"0c»Š?ïÉ,¬†[N?½'ÛPÃô?{i©«¤Lë?½'ÛPÃô?ïŽÉÓ·çQ?ƒ-Ë_F£?ŒM‹ěš?ƒ-Ë_F£?ïý0pë?%ïr¹³0?6|€øÿ?%ïr¹³0?ïög3|Š?Tx±›Y¿?S1™m‹\?Tx±›Y¿?ï3ʸ–ž?²—fÀQ´ì?™†©4–1?²—fÀQ´ì?îÁUÑ©è?›ëPd-?£ïꤝ/†?›ëPd-?ïŬ»›ˆB?v¯jüw.;?})¢Dɱ?v¯jüw.;AGN3FGL J0505.9+6114@b¢¸¾øγ@(0¶â—À:òÿf}À; ºö
´¿ñçêc5¯@(
e‰œ¡@;À n ?ìŠb=(¿é¬l'zk¿¸'eŠzº¿å5¯CéAGNbll@­¬*=p£×PowerLawNVSS J050558+611336?ïÿ˜Éåç¦?à]z$¡?	ÍuÍŒ×?à]z$¡?ïÏw˜N&:?ˆ°mÈ9Òû?xD3ã;·?ˆ°mÈ9Òû?ïéÉ#cÌ?[É÷JR?f6܋µÄ?[É÷JR?ïÿªø1I>ûþÞÚ΀?AôÖô_>ûþÞÚ΀?ïÿsæ#,?ñ™BI…?¢þI¼‡ ?ñ™BI…?îèo"i\n?µ}–¸ü{à?¡yÊF %?µ}–¸ü{à?ïã°í¯V«?qf8ƒ&(?lO1ì½?qf8ƒ&(?ïýôݍq?-kfGüj!?0Y2ÄK?-kfGüj!AGN3FGL J0506.9-5435@pf¸À>-ÀBbë@UZ¥À9n?"zM¤À;P9Ø?çÅ
uÀf@ð»"k1?ù¥Ã P­m¿î[þ÷tô§?ÇÁXXg?²W\PT¿ØÞR—bÄAGNbcu@´Œj^5?}PowerLaw1ES 0505-546?ïû.øƒ?@ŽÖÞMǗ?CDû[²?@ŽÖÞMǗ?ïºzdA•n?'?F†?afæS²‹?'?F†?ïÇUxœ7È?x½lP˜ñ>?|UCÔ@3¢?x½lP˜ñ>?ïŽ>Sš(W?oÈ·<n4?Œpk'4Z!?oÈ·<n4?ïò˜xSÆ?U1@Ï.û?ZÏÖåe?U1@Ï.û?îL>Yü?¸pºWá/´?«>û•5?¸pºWá/´?ïp²\UÈ?|ÂjÀŠ—?'é´}åLå?|ÂjÀŠ—?î°F"ík?•.p)(…?¤û–µtÒ¡?•.p)(…AGN3FGL J0507.1-6102@pæ}ÀTïFÀBtߥíeÀ8ä(í_ŒÀ;ª3Ž¢Å'¿nyJè³=@ü^h–'@%ҟʋ)¿ç¬DScv¿¿åý '®¿çøbí¥¿éø^i¨÷AAGNfsrq@'…
žƒä&PowerLawPKS 0506-61?ïþmº¦?-'³/J2Ÿ?)."³ÏFð?-'³/J2Ÿ?ïʖ¿ÓÑ?'Ÿ¬É›@Ã?z´ '_¸?'Ÿ¬É›@Ã?ï¾ìÉä²i?€Í÷˜ ?€D͍Z§²?€Í÷˜ ?ïú®b厡?0ÂJÆg?EFsraž
?0ÂJÆg?ïýä#P?84­¿œ¼"?0ßÅ ¥/?84­¿œ¼"?ï=^®H?®Îێ¿G"?˜T**Ÿ0Ÿ?®Îێ¿G"?ïiÌt.Èb?'˜q‰/>?'Æqz&óÆ?'˜q‰/>?ï×ɼ÷î?fg'"ƒO.?ty›8áa?fg'"ƒO.AGN3FGL J0508.0+6736@aùÖ`^åi@/È)?"j†À8CÕAæÀ:¿Œž"#¿Ï'Ÿã	Ð@lŠQýù–?ø]q?ˆV%¿¡âe+ÓÿἋw¤¿¿ÃlJÎQÕ¿ É^¶ÍAGNbll@¹Õ³÷ÎÙPowerLaw1ES 0502+675?ïþ™\¡°X?,®üT_ƒ
?&j8Cè¬,?,®üT_ƒ
?ï×3š®Žì?€â`‡W?tf2¿eö?€â`‡W?ïQ´ú·Ûh?"ÁæShh?•É`¬t.ÿ?"ÁæShh?ïÿdêîÔg?U3ŽÀA?bšJá?U3ŽÀA?ïýõJ´?@Û9%S_B?7˜V]—ƒ?@Û9%S_B?îàr—)ÛN?´ß®Üðc?¡ø֑­Î?´ß®Üðc?ïà
ÏC?‡|_LØ.?~/ñ"åRe?‡|_LØ.?ïýW'Ÿ:ª?2L¬='ûf?5Ck‰9†?2L¬='ûfAGN3FGL J0508.2-1936@kŽ(`ܹªÀ?0Üà@GÀ:o4bÞªÀ;ð).ˆª?éK×V5
J@Uµ(Á?P@ÿ^@}¸?ÔdQ^þyS¿áòÆ7‡¿åGQ¯Z¿ïÿf`˜W`AGNbcu@ŽMškP°òPowerLawPMN J0508-1936?š¸±?€=ë?ŒX™X²òÒ?€=ë?íñ°7{þd?®f_ä¡?°r~AúK`?®f_ä¡?ít 6? ~ŠòÓ?Ú?·ü_ê#ßS? ~ŠòÓ?Ú?êö"¯ZS¼?š˜Í¤Š¤¹?Ä%íB–±?š˜Í¤Š¤¹?î­ü¦óä?¤<éÏÄ?¥ 5'yâ?¤<éÏÄ?äÝÇ(sÄ?Θô;&?ÖDq¯Þx?Θô;&?êhñî;Ôº?°¦»Ø«Ê?Æ\8G­?°¦»Ø«Ê?×É3cr]?¯k;ImŒi?äfNyÆÒ?¯k;ImŒiMIXED3FGL J0509.3+1012@gëý`éNäÀ1?Ê ¢¢WÀ9"Çë¼|À;Vj3z€Ð¿µÐF¦"C@#ȶ@zÎ]=s¿çÂR6ôe¿ç?lkQ÷¿æ3–òí•<¿æÎ8˜ÞïËAGNfsrq@"CÒñ©ûçPowerLawPKS 0506+101?ïþ'Ù¥½?$ÊÚ¯J)Ü?&Ògfü™Z?$ÊÚ¯J)Ü?ïÌÒÁ@?…$‡y"Ç?yó½§Ó?…$‡y"Ç?ïáÒi§A?fÊOAû-Î?n-ê‹Yþå?fÊOAû-Î?ïñst'›?CU$ ŒŸ=?]ÌêßÉ]?CU$ ŒŸ=?ïú}ík¨Æ?IÝÿ­Ý»?FKÅÈÌ?IÝÿ­Ý»?î°¨¼Áå?³Lë``½Û?¤õtA–©?³Lë``½Û?ïp09X¼/?eM«'<?'ùøÏÁ/?eM«'<?ï[%ÄEûÉ?ÔݱZj?"›Guˆ¸ä?ÔݱZjAGN3FGL J0509.4+0541@hlë têŽÀ3 ¼€NnùÀ7YˆêíÀ:¬ß06)?תŠm+Òl@70BèÞ@Kù€_
ý¿Ü%<`¿š¿â¶‹AèÜ¿ÜNŠê ½¿â-ZfÜ`œAGNbll@–y\wškQPowerLawTXS 0506+056?ïþËèÔÈÍ?#÷bê\\ÿ?#At¤mÜj?#÷bê\\ÿ?ïÏ;oä?‡‹J<né?xbHTñ‰œ?‡‹J<né?ïÏõd}?}	2ƒ>E?xqh~í¼?}	2ƒ>E?ïþŠŒ,ëé?hÝ°Wù2?'W9»ŸQ?hÝ°Wù2?ïüûø£.2?7y]ãìMÖ?8 9Üy€»?7y]ãìMÖ?ïjj8"?²4'_¼É·?ŸÒ¿4p»x?²4'_¼É·?ïÎY†Gñö?'nïxP¥0?xÓ<»
Å8?'nïxP¥0?ïü6†=¶?6m…¦äN?>Kγð"º?6m…¦äNAGN3FGL J0509.7-0400@iæàé´À8gÀÌäJÀ: È{.tˆÀ;«'Ýãu†¿¼á'Ô'¬@
Æà#Á¦?úaäa\?å6y8Ñ¿à$«œ3ð¿–Ä`X™¿´žD—<OÅAGNbll@Á«õ$ÝPowerLaw1H 0506-039?ïþï0ê?w
‡5?!KF\Ö?w
‡5?ï×ñ
Ī?'eû;.+?tzœû
9?'eû;.+?ïÅë?º¼:?~$Ècgø?}
`.PŽÐ?~$Ècgø?ïû¼(ßó?,†º¯5$Ú?A†"×®?,†º¯5$Ú?ïü³ÍÑQ?;õkRù!¨?:g¹tß#?;õkRù!¨?ï<¼"ó?¢îÔÎÖ?˜hm Ä¢?¢îÔÎÖ?ï©´9ÿ€?…IqÊ-ò?…'üg1L?…IqÊ-ò?ïìvÓÆç?XëÙ8à+,?c‰+û@¤?XëÙ8à+,AGN3FGL J0509.7-6418@q$·@=ݱÀAš†@ €À: s,G‡À;ä"i·S¿¿Ú4ç
ï$ï@§E¥¦˜0@wœ'"¿éêþí¿ä¦¡H:¿â\:$áXB?µú''JVAGNbcu@¦Ót¼jPowerLawRBS 0625?ïÿ¬Â|?4!Šëȁ?"Ò˜œãz?4!Šëȁ?ïՔG'åU?ŒHû'¨øm?u5Üp,݊?ŒHû'¨øm?ïêÌv)–Á?k?½ú[Ú&?e3‰Ûèžç?k?½ú[Ú&?ïÿ‰­¾>À>þð>]‹œ?
" ›ZÈ>þð>]‹œ?ïÿ£a¢?~G¼e[Á?'¦*ͧÛ?~G¼e[Á?ïk»{|ß5?¢{îU6&þ?'ˆ‰"ál?¢{îU6&þ?ïèÙ'¤Þ?m7¶Ytb?g&ØJ)Î?m7¶Ytb?ïùæ—4uº?CÛ<¡ìFÒ?He¢täÍ?CÛ<¡ìFÒAGN3FGL J0510.0+1802@gû¿"ÿ&À)‡LàƒböÀ8ÀÂã>ÿÀ;7&ùz«?åMƒ2©v@øîÀ½të@F§ msK¿ä¿Ÿ±Fð'¿åîç²è[Z¿ál;ò–ØA¿ë—6Ã5ŸIAGNfsrq@Œž^Ñ·PowerLawPKS 0507+17?ïüÑQ8NH?5ló·ìï?9uwvê"4?5ló·ìï?ï¹sK­?Œ¼6Òz
Þ?£-FS.M?Œ¼6Òz
Þ?ï•ö#)È?ßgéâ?Š'w?ÜÌ»?ßgéâ?ï¶"mÏx?]…‹¤?'w£,J ?]…‹¤?ïöéOr?N&Ï}×b?R-é$¨í?N&Ï}×b?îQL´õ¦Ç?¶*PTŽõ?ªë4¯É¬"?¶*PTŽõ?ï	$ee
?–°C‹7Y?žÝû{êdÁ?–°C‹7Y?î"|ÀÞ?'4j¥A@Þ?¦Ïx4ÛY!?'4j¥A@ÞAGN3FGL J0512.2+2918@eõW´Àx=`2Å¥À9®§â1¸àÀ;9WÒNìÍ¿Ûb1ÍF^"@{——᳏@@¿ ¿â@^xõùÜ¿ã2»!1[ ¿ë"j2xοå~¶0u‹AGNbcu@†½'»0PowerLawB2 0509+29?ïûôÚÜ?PÉ)÷Ä ð?@/œÙG¸?PÉ)÷Ä ð?ï·õ~¦?Œ2·x¬Øô?' zP¬?Œ2·x¬Øô?ï¦=Ƭn«?ƒÔÏI"¦i?†pŽQt¹Q?ƒÔÏI"¦i?ïü'ó9?(Ó»‹Å«•??öÁ÷‰tk?(Ó»‹Å«•?ïÕ°—s4ç?€"˜9&…?u'´+˜˜"?€"˜9&…?í÷´€>™?½LF»·aè?°G"\Ùò;?½LF»·aè?îË;cóe?™ï]‹ðec?£LI½_Ý»?™ï]‹ðec?ïÁ?B‹ñ?rîTæÂ?`^Úï?rîTæÂAGN3FGL J0512.9+4038@dѾÀ//˜?íJ =?ÚÀ9Œ$ôÀ;[a8)<9?è6âGæÒ@"WJê‰÷@͋?cÿäz±|íÄó¿ÖÔ»Ðóo¿âX[œ'¿ãäâ^É'ëAGNbcu@¢'!ä÷eþPowerLawB3 0509+406?ïü@eJÝt?9ep–ñÁŸ?=ü×6ØS?9ep–ñÁŸ?ïqZî¢I?žÉÄ-¾à?'Ô¢;üó?žÉÄ-¾à?フ›ëj?u·5º·?€|\âü‡?u·5º·?ï*é¦ÞaÜ?pEÖ¦ýɲ?š¢Ë Ä(‹?pEÖ¦ýɲ?ïçI="=Ã?gÖÒ/pY§?h¶Â,‰m¡?gÖÒ/pY§?ë™c¨Ï?Äø¸8E?Ãí›Âq\Â?Äø¸8E?îÕ'çЉE?œODio
?¢­†g­?œODio
?êÙà§Ü8·?¡@Òln?Ę}`%?¡@ÒlnAGN3FGL J0514.4+5603@cBß72œ@$»ÁÎjÀ9|5Om&À;}Q›Ô}¿ë¼T2öç@œ,µj°x@·Ñ?Î!6¿è¡ø‹žþ¿éŸã*cÇ¿æƒxÒÇ-¿ãxÓ~ LšAGNfsrq@y™²êòPowerLawTXS 0510+559	?ïÿ%=brL?ËݕEü;?XP`ãÊé?ËݕEü;?ïËú¢P«?‰nág¶?zx';B³?‰nág¶?ïÞ:	*?qûEA»Ô²?pâûdÉ.?qûEA»Ô²?ïÿ¢Ð¤ô?7ýMæ?kå~Kº?7ýMæ?ïþ]ÌlˆG?/<³þ¿&è?*#7!8$?/<³þ¿&è?îñ3X
ò¼?³'dLøچ? ìÊ{á8D?³'dLøچ?ï¼%gÈ«?€M¹üÐrŒ?€ö¦w7?€M¹üÐrŒ?ïð›Ê‡‰]?WTDö33m?^ÈkK¢õŸ?WTDö33mAGN3FGL J0515.3-4557@ow•@%NÀA¶ó=<¡À:(»ìª¸¦À;›ÕÎÔ
¿©åD²Ÿj@/ÑËdAô@p@.ï,¿éÝ"®Y¿Ö×c©ž¿ç±"£ï×σ3ÒAGNfsrq@"PÅÖ8†YPowerLawPKS 0514-459?î8*÷$,?ª•ŸßºØ\?¬}P‰kŠN?ª•ŸßºØ\?ïÌåÁX¨?ˆ";èY2[?yO1Ä?ˆ";èY2[?ìW˜AC°ô?¦!?2ùZ'?½C=õâxc?¦!?2ùZ'?ïš;PÊ.?o÷È-¡?‰q+×ÃL¦?o÷È-¡?íЉ'1–?²/¸›Å§?±{·[Ï?²/¸›Å§?îÀƒSd´"?®†ü1_
·?£÷ÊÇ!Ñ?®†ü1_
·?éÓÍÜ{Ó?²ôÁæ`??È°Ë Ž¶?²ôÁæ`??ê˜8'\}H?¯xysÀ^X?ş¶Ž
ß?¯xysÀ^XAGN3FGL J0515.5-0123@iY,Ÿ/ېÀ5Þó_ތéÀ:™`sÞ.À;¸õ½†ß?èkÅd½^@
ch/>\?üÆ`Ìôe?Ôq'ð$b,?æ5ÓL rš¿ÐÙí­Ô¿äy¼*øÉAGNbcu@µ{`IQƒPowerLawNVSS J051536-012427?ïýºš½}q?=¿&c™T?2+)Š¤‹?=¿&c™T?ïˆA¶s? ˜
úå!?žn÷À§‹±? ˜
úå!?ïÔzB'J?nØÁNs¾?uüÂóUÙ?nØÁNs¾?íÔº€Þ¦ƒ?ËO]Ü
J?±Z+û0g?ËO]Ü
J?ïñÊG·N¶?_	$XZM>?\kpìBõ?_	$XZM>?êʆöÌ?Ä
¦'yº?ÄÕä$Ϗ—?Ä
¦'yº?ï™M¯V?†æÑÓZG?‰¬¾ÉÛª?†æÑÓZG?è"o,¢d2?²¹3¹*Å?ͲCMvo7?²¹3¹*ÅAGN3FGL J0515.8+1526@gwÿ´€¦À*"ÚA)•ûÀ8Ϋäõ¸~À;.Àp÷Í¿ò±ÞÇ;@$M˜ö\@ŒÐ¿u¡B¿â׳Í2´¿ãtsè/(â¿àèÑÝz;¿Ùø1<ìxAGNbll@ z±Ä2ÊXPowerLawGB6 J0515+1527?ïüún	Œµ?1í½pêV?8,'4n'G?1í½pêV?ïɼWð½ÿ?ŠLw"9¢?{!Óët4µ?ŠLw"9¢?ïÖ$cì?uÉú¹/é'?týí´T'"?uÉú¹/é'?ïÿµ P>ûz«­ƒ…5?·þo™	ø>ûz«­ƒ…5?ïùãz}
Œ?A¥É¯X6?Hr6šè?A¥É¯X6?îÃer?°q;4ªÒ?£É¨á"SÄ?°q;4ªÒ?ï›ø'ß?ŠsÞµ\·Ÿ?‰8ÁïLt:?ŠsÞµ\·Ÿ?ïûp«'¥O?=ê²-"®½?B=SÒª¯?=ê²-"®½AGN3FGL J0516.3+7351@aSÊ€à@3Æ"à՘MÀ9ò¯ÑêBÿÀ;ÐùyÔt?òá']
9@‹³÷ñt?ÿu«€vÝØ¿åM¤éXôŽ¿èôA¸Sm¿ÍgrÓº°H¿ÖÊBÐpUAGNbll@ªúu%FPowerLawGB6 J0516+7350?ïöD=عÑ?WT½yÏ ?Sw"Ò}\í?WT½yÏ ?ïSÒ|(w?ž=RâI7Œ?•…°Þ)%?ž=RâI7Œ?ïc}'¯Ì?@K‡ƒe§?"O¯Dðƒ?@K‡ƒe§?î缔ñ>F?ƒêS~ØØ?¡"6®Xf ?ƒêS~ØØ?ïöj×ÂÓ?Vì
,ïL?SÃ*š±êB?Vì
,ïL?éÚ½ ßÞø?ÆÜ`ܗMÃ?ȕ	|€"?ÆÜ`ܗMÃ?î±=Cú£? G3 _i?¤ì+Á1µ›? G3 _i?ë¥ü'H}®?­U ¬"‰o?Áh
¶Þ	F?­U ¬"‰oAGN3FGL J0516.7-6207@pø6ÀP½ˆÀAaG P À8/›fù3]À;JbýüÁ?åãÁ¦(U@pyà@)Á'°—¿ÛN{Òοãhxt…ãÚ¿à–€Ï7$¿æ]º,§ÜAGNbll@ût¼j~úPowerLawPKS 0516-621?ïÿšm1º@?¨£Ô®ˆ?	d¨«Q!b?¨£Ô®ˆ?ïÎ	¹?ˆ@¼j.?xþ{%OAÊ?ˆ@¼j.?ïè"vâ+ü?j¤	1?glˆâº¼S?j¤	1?ïÊ­ý"?_o9 ˜ˆñ?z©q-i÷?_o9 ˜ˆñ?ïÿ5¸¾,?=
9$Y5?I'ò#?=
9$Y5?îö0i1ûX?²É¤8kò»? œùjL•~?²É¤8kò»?ïÔK@Æ?~£ç¡Êuœ?uõZ_œó–?~£ç¡Êuœ?ï
ÝÂF¾?‹¹ çcù?ž¤G°^PD?‹¹ çcùAGN3FGL J0517.4+4540@d^\FR@÷QÿÒÊÀ9ËzdJ,tÀ;UÂ%©Ý´¿ä>ÏôEÑ@hú?v¸@°IÀheo¿ç²¥4M¿è¢9`ýN}¿àî«ÌÌ÷À¿è3MU%ÿÍAGNfsrq@9¢3œ¿PowerLaw4C +45.08?ïÿåÑÃÆ>å\H¼jˆ>êðê	½c(>å\H¼jˆ?ïÎ'®Þ¶?Œà¯ÓxÕ­?xìs«PTÇ?Œà¯ÓxÕ­?ïív°¥>?g"D4´×?bø‰¡R¥?g"D4´×?ïÿâ^Â>Û!ìq}þ>í¡ˆ¾r˜ñ>Û!ìq}þ?ïÿæ¸jx>åËHgŸ>éH8n':>åËHgŸ?îÚ8m"½¿?­Ñ½fAAX?¢\y(?­Ñ½fAAX?ïã¸Ø_cN?rŸˆÑâ>±?lG'‰?Z?rŸˆÑâ>±?ïÿOn°ÀZ?Á‰L
Ûb?%ç6"?Á‰L
ÛbAGN3FGL J0517.5+0902@h0à?pXXÀ0)ÃÀ´–À9Æb‹æR°À:ùŽ,~
¿ä¤¤Ù$R@Ë°…ni@b»q"î?黎W4ÍÆ¿ìñ÷MB·¿Û­ðÂåC¿áä|í͉œAGNfsrq@¦.ã¼ÓZ†PowerLawPMN J0517+0858?ïûšA׈4?O7Wè5ƒ?A–ønЇ?O7Wè5ƒ?ïÌUë2Ø3?ˆ±òëjRÌ?yÕ
`dšc?ˆ±òëjRÌ?ï>²‹`¤c?'Wä1\2J?˜)®'3¥?'Wä1\2J?ïýO¿?"äˆu‰MA?5'#8Œ?"äˆu‰MA?ïï–~°•?jmzÍÀ¯?`i£)¢}?jmzÍÀ¯?îÚ~
Žº?²O,*ÌÇ?¢X,¿Fj?²O,*ÌÇ?í܎ז!?¥')_T6T?±ӊ5ø?¥')_T6T?ïê%îQ+í?\̐S­ ¿?eڐ—ƒ'?\̐S­ ¿AGN3FGL J0519.2-4542@ooý¿HÌÀA]›ÿ¥g-À:QÈI°MÀ;qÕÉːÀ^+¸ën@R#½Iw@ááÀ¤ËQ¿ãMsjƃ¿è;ԓ¯cŸ¿êÛ¿Z½¶¿Ð²­3KÔ6AGNrdg@"ÁµÂ\)PowerLawPictor A?ïÿ+ٚ?#çؙSÉ?"ÊŒ(ë*?#çؙSÉ?ïٖ,M³?…¨+"è»Ò?s4òHÜæ"?…¨+"è»Ò?ïÈõõŸ#?p2±LÐ}…?{…có>®?p2±LÐ}…?ïÿÿê†q>f<eŸ"±>e7¾¬áñ>f<eŸ"±?ïþ-;'?r?3	³ùb?-,C
'b?3	³ùb?ï`ìïW?¬Î!cȔ?"íÿ¤ã?¬Î!cȔ?ïiÃ7Í¡´?êú½Ôj?'ǘý´ÃŽ?êú½Ôj?ïÿúÌôÙ>Ðux>a6>ÄÎí'lí³>Ðux>a6AGN3FGL J0519.3+2746@f:" ³Ô®Àá'_Á0·À9Ó[&—C~À;iï‡â¸¿ôËó @݅6‹,n@¤y¿^¥'¿ìS«lfð¿âö:qÆ}¿ÙÝWu9¿â~'ùZAGNbcu@ jffffPowerLaw4C +27.15?ïùڐɀ+?TGE·(t?H•½ë·?TGE·(t?ïµ®:e?ÙÜå$°¯?'"qYéO?ÙÜå$°¯?ØÎÁL?…´L´tÍ?‰\‰Ý}¸×?…´L´tÍ?ïÿ˜²F—G?
·›hí‰?	Óg2ՙµ?
·›hí‰?ïÑœLž·?€`(¡P?wx1ÜpT¹?€`(¡P?îl$Î7þA?´ÅÕð^¯?©=³€ø?´ÅÕð^¯?î‰l³1›.?5Ÿk=?§i4Ë.)?5Ÿk=?ïúGêƒ?C'ë{°1?GÿÏÀ"?C'ë{°1AGN3FGL J0519.5+0852@h=쿱[WÀ/°¾|§ñÀ99{*BÉ©À;šþô?ùÀZ*ÃÍö@'´#lÂ?ÿﴀ¥¬Í¿Üû¾Ê"¿æWdØi/'¿è?ÀDb¿ïÿ¾ú¤™AGNbcu@G­VLogParabolaTXS 0516+087?Ò/¢÷ޕÄ?ȤŸe̅?æè."µ?ȤŸe̅?À›ïŽ‡†‹?ÅÙHNVó?ëÙ^]?ÅÙHNVó?â*Þ6<ä?´'4ÿåI?ÛÙªC"†8?´'4ÿåI?ÒvÏm:I?¦'Bچxô?æĘ|IbÜ?¦'Bچxô?§úxŠ2üà?°´ÊŠmÐÀ?î€Xw\Ð2?°´ÊŠmÐÀ?Ÿ­'¯P¡>?¬f
µ|?ï"r…zö?¬f
µ|?Õþ˜*|A?¶GÄzBç0?å³ê±Aß?¶GÄzBç0?¦ýâ«ãQ?ö;ô~s?î!߉›?ö;ô~sMIXED3FGL J0521.4-1740@kuNóÀ;•sà¢l§À9ÇquŽ!–À;Áó™À0¿ø›«–ò@ÓtMéÄ@nó€jÉx¿âBå'Ñ++¿çѪÒ'¿çi ÙŸŠ¿Üç¶vãÐäAGNfsrq@†È_oÒóPowerLawTXS 0519-176?ïýÃí«¿?@hmï–Lh?1à'˪°Æ?@hmï–Lh?ï×¹lj-é?'ì<À¼O?t#Ièu¯Ž?'ì<À¼O?ïÅI,2§·?tMùAþ²¸?}[iòZЄ?tMùAþ²¸?ïÿדF»ž>ì†
5îÕ©>ô6qtŸáz>ì†
5îÕ©?ïõè"/Çe?\"­˜÷T­?T.ø¥É?\"­˜÷T­?ïG×Bz+ž?§ù8:®ý"?—©ÛTQ?§ù8:®ý"?ïW6ºž™U?+^@­8?•(±T?U?+^@­8?ïûCÑ¿r?Cþc"«ºè?Bð¼ŽYùU?Cþc"«ºèAGN3FGL J0521.7+0103@i)rÿÑÜ×À3T‡`±ñÀ:5:¯(wÀ;š#;nk?ÏœÓ+¼@pÁFóµ?û-€H9Ö?îâw]•Ä¿Ó"¨)Ãf—	'›â¿ÇEnbøâAGNbcu@ºˆ²@·€4PowerLawNVSS J052140+010257?ïÿA!ć? mÏÙå§?ÛÀe¬Ý«? mÏÙå§?ï»Þ§Y'?"Ü«?<	?V$Ì«{?"Ü«?<	?ïääcÊÞ>?`Ùl	ÁßY?kœZ=Š?`Ùl	ÁßY?ïúå5==g?,{{¬_Î)?Dk*9«€?,{{¬_Î)?ïþ$÷ÂU?+C9ĎÏ?-°†ÓŒj?+C9ĎÏ?îçTâIO™?²(·mwÏ0?¡Š±Ýþ»l?²(·mwÏ0?ïېÏ=ñ?tÀú`Í­ð?r7˜Æ[?tÀú`Í­ð?ïñÞzQÞM?MøÇ]q.ý?\Czöw?MøÇ]q.ýAGN3FGL J0521.7+2113@fó'àÀ!gž´JÀ7LªÓ}ÁÀ:l²oStò?Æp^'ê@ëH>³?þĤ_E_Ü¿ÜÙ©Þ¿à
õò"Žp¿Û°Š¡Ú¿ÜSóÉAGNbll@ /ß;dZPowerLawTXS 0518+211?ïÿ³ÕW?p›OWX?i~[`"?p›OWX?ï¹Éê5È?'N¯ùGù?…‹°ýØ?'N¯ùGù?ï'üÉ-Ÿº?xûJ0?‹€Í´˜s?xûJ0?ïÿ"ȁ0?	ɂܟk?½'‰óþ?	ɂܟk?ïühDL?;…<G/†?;"½"C˜?;…<G/†?în*;Nü?¸€íµ>†?©\M²8?¸€íµ>†?ï¼Ô«#Àá?Š…1̎‹	?€ÊÕ-ÈÕç?Š…1̎‹	?ïývK¸?/{¤4»?4Oˆ5´´?/{¤4»AGN3FGL J0521.9-3847@ni>_·¼À@­? (ÿÔÀ:?³~G-¼À;Ç?QN§-À¬âF[®ý@^VYS†@… êÚ¿í=ÌÍ´ºn¿áƨR⌿äì~9R`¿à".¾¯SAGNbcu@"Od?åÉPowerLawPKS 0520-388?ïÿéÎƾ>æaåÁM5>æ<'Â>£>æaåÁM5?ïÙ]kóÄ?†¨§>ðA?sQJh¸‰÷?†¨§>ðA?ïÛuËÍã?q6³´o?rE3ÛkJ?q6³´o?ïÿÿú+è>Q¶Ú›™f>G]ê›0ªd>Q¶Ú›™f?ïÿä‰#w >í|\
>ëw?ÑÚ>í|\
?ïAÂÔ6µ?•Ûzø_Eâ?Œ/=3âè?•Ûzø_Eâ?ïÁ@>ßcÓ?^/èPbû?_à±úB5?^/èPbû?ïÿÿmo*k>˜Jñpô>'T˙G´>˜JñpôAGN3FGL J0522.9-3628@nð`»+»À@[ò¿¥œÝÀ7ë×TLÀ;$†îœ*n?ðZYŠµÑ@æÑZÑ@/hDq¿â§ÝÖº}¿ç8Á5¦\¿ç%]Àƒ¿ä}óKoG¿AGNBCU@t•$ÝLogParabolaPKS 0521-36?ïÿX¯]j?å?Æ?êX1?å?Æ?ﺎ¤ÑŽ±?•ö8éÆü«?\V¾ÏÎ?•ö8éÆü«?ïJ0Ä]?‰1n`PÊ?ˆ­\¾¼¼?‰1n`PÊ?ïý¦GH¥?øÃ^ÓÜï?2ÏßM'îž?øÃ^ÓÜï?ïþÔ®Iˆ?&÷wȜè?"¾ì®Í?&÷wȜè?ïD82¼?« 9:ÇÎ?—|y!y?« 9:ÇÎ?ï5#ÎÄÒ5?"ûºƒÆ‰í?™[†*ÕUW?"ûºƒÆ‰í?ïû°²1b?<5Üû¬b?C<JÕWˆ?<5Üû¬bAGN3FGL J0525.3-4558@o}Øÿu–…À@Ùr 0ŒÀ:VHø"À;Ù®&ïX?âÁ©\t	@Ñc	/ª@œôBp¿åØ ¬¿â	õH…Ä"¿×suéOY¿í€±b°qAGNfsrq@ž"¿—$tTPowerLawPKS 0524-460?«xá‹?ˆŽIª$?‰Ø(¦ÕQ?ˆŽIª$?ï«{;éå?ÀáQ×?…!0þÚÎß?ÀáQ×?î.Çg¡éŽ?™×SŸ¼³?­‰…ág?™×SŸ¼³?îé"vzcQ?€G€¨Í
U?¡g¸"ê.ô?€G€¨Í
U?ï F·Ê\?›ÑkñTfk?›üW,vPu?›ÑkñTfk?íü $"I?º.Ã{¯?·˜þ¸?º.Ã{¯?쯝@?«0æ"Íú?º‡'3&?«0æ"Íú?éYgX…?´zí?G¹^?ɾšbŸåí?´zí?G¹^AGN3FGL J0525.6-6013@pÑ̀CRÀ@ïÇÿÞrÀ9•üÁ‡mÀ;zšéû±½?ñμI¢á@EpOô4?ûžŒÀmBù¿Òæëˆ
X¿Ü2Ýð-¿"œb2
zi¿áD‰8ð®ÌAGNbcu@²C!‰7KÇPowerLawSUMSS J052542-601341?ïÞ3­è—??l—†!ø7?pæ(ù&|«?l—†!ø7?ï ?B¶?'ž{FÃ?‡ð/Uí˜*?'ž{FÃ?ïH§ë…¹W?÷åle`?–ëHÕ(?÷åle`?ï·W"=?|f©ä‰¼¶?ž	'"~T?|f©ä‰¼¶?ïÁI\šá?y–Ô‰ÙÚ?[{ÆãÅ?y–Ô‰ÙÚ?ì÷†éàü&?Á\D^y?¸CȳàL?Á\D^y?îc¬3
?£
UÊ[=?¯ßÅ<ÏX?£
UÊ[=?íÀ#¹:¸?¡!|l]š?±þçœ[ë¹?¡!|l]šAGN3FGL J0525.8-2014@kÙq`•l
À;ñ Á¬À:[ìSzÑWÀ;ß:ZMS?–PnU_È@zû¸G¯—@€V@(¿×®éö0üÖ¿á¹u«dš¿×ˆ€º¿èü·•FèaAGNbcu@Ÿxi­BÄPowerLawPMN J0525-2010?ïÒ
Îõ›ù?°Ì'€7Ø:?vùm$¿ª?°Ì'€7Ø:?ïÇ÷'?Ž&¾} 3Ÿ?|qýà"1?Ž&¾} 3Ÿ?ï´@ÿ¤n?ˆ½X'G¨§?'ïÀ&ª'?ˆ½X'G¨§?ïêÁN÷?Iðð›ó‹ß?eú>à'€ë?Iðð›ó‹ß?ïù²-º"{?P!"F9/¥?I7Iߒ…u?P!"F9/¥?ïDÙf
P ?¢wM
í\?—dÓ7vÄ?¢wM
í\?ï`ôl×wS?"Á»Píf?"ár^1ݟ?"Á»Píf?ï\Û{øZ*?ƒŽÏ"ùË?"d{ÍP·?ƒŽÏ"ùËAGN3FGL J0526.0+4253@dÔ_õI@Ã×Àâ¯À9\sв4›À;SÕ™êø?òmJ(B>i@óa4Î=æ@{ðà}XÆ¿Ùm¹,˜­¿êzôE•¿åÌ
ÏmÞL¿ïÿàL¨ÇAGNbcu@†Š;?¦ÞüPowerLawNVSS J052520+425520?ìo@ç¯?¼¢³.ý)È?¿ì‡Mø…?¼¢³.ý)È?á;îJBeÎ?ÇïCvÕõ?݈#k{4e?ÇïCvÕõ?êV§4?€?¬Ð³M!º?Ǫ¥c/ÿ?¬Ð³M!º?åQNêŸ? @ç-¤'—?Õ]áb*Â? @ç-¤'—?âr)?¶µ?ÏèBSâ€=?Û­ù€'•?ÏèBSâ€=?ÂòV­š?ÅÌDbkÁ*?ëC_ªyT™?ÅÌDbkÁ*?à¹~ÁŽ~?»Î͜Å7?ލ}Äã?»Î͜Å7?ƪ˜´07š?Ÿ©;ëAÅ?êUYÒóò?Ÿ©;ëAÅMIXED3FGL J0526.2-4829@oßU>öµÔÀ@àn¿Ñ;ÇÀ8Êû¡ÌnÀ;\¾óÆ5Ú?Ó¼0ýMô@N˜|äG@NR@i§Ž¿âÓ»Ôàu)¿ãÏ¡t?©¿ã"¢3ž¿ç…l1g½:AGNfsrq@'àXÇâ'APowerLawPKS 0524-485?ïÿ(ÝõD?{Î5{§ý?ä\|/À³?{Î5{§ý?ïÎ'š›Â?'â=Z%%Ù?xì2˜V—?'â=Z%%Ù?ïäzAÔO'?pQ­l>R…?k…¾2ND?pQ­l>R…?ïý¯²µŸ? -F.íu?7êC§¹×? -F.íu?ïÿ`Š6¥?œ¶ç¡ñ?þ	±>?œ¶ç¡ñ?ïX6ŹÞ?ª5!BA"_?"ù'HÄ?
?ª5!BA"_?ﰃ-ªç?…?›yØ.?ƒß?ò-ŒZ?…?›yØ.?ïô§‹u?IÕל7?V°ê*&R?IÕל7AGN3FGL J0526.6-6825e@qm~KZÀ@lӀE4½À6_MkÝyÀ:?æW¸Mº?þOI"H¢@èVÁèb@u°Ÿoœ¿ß¾Nî÷ð¿ã7we'+¿å³ß@¿äÂôÁÞ\AOTHERGAL@xÅ&þqŠ‡LogParabolaLMC?҄c"wÍ?Ë>ª=9>?æ½Î5òD?Ë>ª=9>?Â`´¸P`b?Ë芩¢â?ëgÒÑëçç?Ë芩¢â?á½Ò(Tw?¶ú+ȺZ?܄[ѯW?¶ú+ȺZ?Áó$Fӛ?¨6
̒2?ë›Ã6îK?¨6
̒2?ÐÌMUÉ5>?Ë畤t®?ç™ÙUea?Ë畤t®?²Î/ñãO?Á>5MrW>?í¦:ê¢?Á>5MrW>?㗱ޛ¥?·öÇÑ-Ì?ØМBÉܶ?·öÇÑ-Ì?—Ÿ|¦|}•?'ÏFkø‹<?ïC°Ÿ3?'ÏFkø‹<MIXED3FGL J0526.6+6321@b"™Ÿä6v@.†þ "ofÀ9úÈ×'šÀ;͔ãQs?è
™"GÊç@hfʺMï@Q·fw®¿æâ?j¤
¼¿ãTR+Š·¿ìJªó€&¿ïÿҁWèAGNbcu@ƒi8ºÇËPowerLawGB6 J0526+6317?ïåqo•s?qÜiOk	?jŽ€Þ
D?qÜiOk	?í¾üøíÒ?³Þ¤¨¥×ê?²7MVò?³Þ¤¨¥×ê?î¾ä±åÇ?'ô
È2?¤´òX"?'ô
È2?꧄µ ¥?š,,·K¹Å?Åaí)}kª?š,,·K¹Å?ïš™ýJL?¥ 
Ý%o?Ÿl¬¾žèŒ?¥ 
Ý%o?àB/ÛÖ?ѵšÛQä"?ß{ IáöU?ѵšÛQä"?래im×Ê?°¾7ÔÍ?Á…žZH Ù?°¾7ÔÍ?Íj"­êq?¨šñ'¼Ì?è¥wTºd?¨šñ'¼ÌMIXED3FGL J0528.3+1815@g^·`¿]yÀ"d²—À:s'7ËHhÀ;™;ÞÓ_Ž?æ5P÷¿>Å@qZRÜÆÀ?úU{?Œ?¢eÉæñ勵¿7¿8Sr]¿ÚäP¨u:Ñ¿Æ¡eÑýŠAGNbcu@Ä,˅¸RPowerLaw1RXS J052829.6+181657?ïý`3؅Ï?1Ê:'¼N?4þ_!Ì®?1Ê:'¼N?ï¡…ðƒ?'h¸‡7Å©?‡½v;/Q?'h¸‡7Å©?ïÔ×·?m<ä|™"?u"r¡³Èˆ?m<ä|™"?ﴆšìÞn?fè)éD¢?'ÞY@Pæ—?fè)éD¢?ïîx±ËQ?`,ÑóéÎ?a‡N§?`,ÑóéÎ?ìwf¦¨ï?Á½ïfy?¼DÊÊ¿†?Á½ïfy?fi?‰;6 ž?Œ9;^E¨?‰;6 ž?î8×±
?›Ë¥†Íd?¬~²…ËFë?›Ë¥†ÍdAGN3FGL J0529.1+0933@hSvÿ:Þ"À*è¬A<
rÀ9fµ¨ÃÙÀ;DBì䚿æ
·­Å@^&ˆó@ˆÏ`zê¿á[Æi¿çœÏ2å[¿ìY "Qº?×0sêwFwAGNbcu@–®Ížƒä&PowerLawGB6 J0529+0934?ïùm|Ò?Sƒöcƒç?K'KÙ]À"?Sƒöcƒç?ïÊ,‰¥õ?‹ÞbÊ?zéü3áZ?‹ÞbÊ?ï¦ìrm"?~j	³e»?†Dã|7??~j	³e»?ïÿç€F%B>â¦gˆMRå>èáo;\>â¦gˆMRå?ï¹²§˜Æò?…'¬ƒ†PÊ?"V=ß|?…'¬ƒ†PÊ?îÃÖC™ø?³WÔq|‡?£Â›ÃÛۊ?³WÔq|‡?îa¥‡—:?ŸÚb#Æ
?©å§†Žœ]?ŸÚb#Æ
?ïý¨‡s&h?6å C%=¥?2»Âõ]&?6å C%=¥AGN3FGL J0529.2-5917@p¿j€JÀ@½i@5z5À:\(^ÃÚ¶À;Ú`S&ÛSR¦¿@
—>•¼ë-@ÿÜ TsË¿èüî8ég¿åuk—RÂp¿á\6°§cm¿ØSrÇ^AGNbll@"%^šPowerLaw1RXS J052846.9-592000?ïÿ]øz?€U ¹	¼?T=òû‡?€U ¹	¼?ïǤÿJÅÃ?"Zî ø³?|-€:PÊz?"Zî ø³?ïÙbMcF]?sUšž?sNÙ^Úñž?sUšž?ïüÁ8¼V?$W_\«{?9ö:õæ—?$W_\«{?ïþ——ƒ6M?'÷ dَ#?&†Š­GhK?'÷ dَ#?ï5'5	]]?°Rsæè¾?™[bCðY?°Rsæè¾?ï ôp™‰î?"Èû£¤?‡Âãç[ôf?"Èû£¤?ïÓ_d$ÓÛ?l§"ò‡í+?vPMËéæ¢?l§"ò‡í+AGN3FGL J0529.8-7242@q¼¿šÏúÀ?×ÇÀ'áÀ9«èYM‰À;ªÔ}›6¿úhßè]vÿ@/€3;@ÌπsÝ¿æ^ï_Úí¿ë€ [ՓƿԬ0ÈÓK ¿èü2•ÿ[AGNbcu@‹Lì <K
PowerLawPKS 0530-727?ïÿÛ$~dŠ>ïÎ_zgðŸ>òm¶y 1>ïÎ_zgðŸ?ïÒb,'R?ŽJ…ì/ìì?vþNôµ—"?ŽJ…ì/ìì?ïçM;>'Ø?v}"Òm?h²Ä·Ï?'?v}"Òm?ïÿúÏÈt>Â%‡™J2>ÄÁ JþƎ>Â%‡™J2?ïÿî0äh9>à*Üs­T>áÎÜÝû—·>à*Üs­T?ïMpŽæë»?ª´¹{­?–Qî²ìµ?ª´¹{­?ïâV¡CÔc?vJ›;#§X?m©^ßç??vJ›;#§X?ïÿÎj9bU>ø^Sïj†¦>øÊæó8T	>ø^Sïj†¦AGN3FGL J0530.8+1330@gëü–þµÀ&‹$£MÀ7ºÇªÀ;ÒÎn|?ýËk[BÆÏ@._@B-¡ú¿âúžrœU¿ç—Áf«õV¿èêPⲊ¿í'H¶ÁâRAGNFSRQ@uHցìÔªLogParabolaPKS 0528+134?ïË)Ú¢€ü?}h˕õ4?zk™qíä?}h˕õ4?ï|µ tJ?¡Yë~Ÿµ?i[÷>É?¡Yë~Ÿµ?ìe‡G¡C ?­
gÖá /?¼ÓÅÂõç?­
gÖá /?ïKÐkµ'?{ñÿù(W-?–Ÿeû a
?{ñÿù(W-?ïš'pŽ?›ñé6ÆØÅ?̦ҶH?›ñé6ÆØÅ?í\Q\
?ÂêåëÆ{ê?·¥v×yƒ?ÂêåëÆ{ê?íh¶T\Åö?¤Poµíy?´ºM]‡ÃÏ?¤Poµíy?î'Ošyœ?˜e¡À:µa?§Û©È;?˜e¡À:µaAGN3FGL J0532.0-4827@oà 6mÀ@g`#VFÀ7F™¦.ÓRÀ:¤"Øi¹?ö¨Y-æ&@0¿»lR?ÿ}•øÛI¿Û¾òˆ¤¿â—:·6¬¿á;—ÇB°e¿å£^™4ç5AGNBCU@ˆ¿¿3‡LogParabolaPMN J0531-4827?ïýàÙ>Ú?2µþ?ú;?0ù6A†Ô¨?2µþ?ú;?ḯ±#+²?ŒÖ	ñÍ5ž?y?'v©7?ŒÖ	ñÍ5ž?臭(¯-?'Ö\-QŽ?…˜õý4¸?'Ö\-QŽ?ïÿÙy$ü[>çGLõ°ÛÇ>óC•Éz…>çGLõ°ÛÇ?ïùϹ*x?IeNI«T?HÁ yb?IeNI«T?ï2s[Ü
¡?²còåRd?™±"Váß?²còåRd?ïûÒì?o&ÖúU?‹Á>ć?o&ÖúU?ïÿì->äÔ>0T>ãÒzu_Æx>äÔ>0TAGN3FGL J0532.7+0732@h›5'Ì÷À+sóþiýËÀ7|äJ7\À:ޖstkã?øVV"÷@ʖpÅ:@¶¤¨ÁTÊ¿á^jL¶"M¿å°?é$h¿ä3Rè°-/¿è6¦¼þàAGNFSRQ@}d2ßP]LogParabolaOG 050?ïýâ6¶?0Óõð.·S?0îQ0ªtN?0Óõð.·S?ï´ûIâÍ?'`OðÉ?'Á-‰\~ì?'`OðÉ?ïÀeda?€A'BÌ|?ÍMÒy³?€A'BÌ|?ïùnzÿG?4eº¹õJO?JFàd¾?4eº¹õJO?ïú"W1¨?GÈՐ;ú?E®¡b²{?GÈՐ;ú?îVÊÚóñ?º1ÈW¥·?ªž#Ná$ù?º1ÈW¥·?ï\0ÿ¡4?"Oäû´ð!?"yàDo}?"Oäû´ð!?ïøö"'•?H0;«'%%?OÐ%Ò>Yì?H0;«'%%AGN3FGL J0533.0-3939@n˜¬B»fÀ?d;ߪ#À9îRŠçO/À;¾ê·™^áÀš®ý®í@A
;|Ù@æ½ÿ|¿×¦¾laÓ¿èØKIeµÎ¿æ*EEPäk¿á_"½'"AGNbcu@‰ÔÝá\¦ÊPowerLawPKS 0531-397?ï݌v¢¾?­é(»Ê?q9ÄàÚÌÆ?­é(»Ê?ïחP¿
A?ŠâoÝ8Í?t4W…­ëi?ŠâoÝ8Í?ÿ=¹?ŠÃꖅiÁ?ŒW@B`-Ú?ŠÃꖅiÁ?ïÿþzÄÂ<>§ªÐC°>¨QÇHûQ>§ªÐC°?ïþ‹íoÀ¾?1z=å]D{?'A(nkh?1z=å]D{?ï5çœË—?±U]n^ò?™C_­ç9?±U]n^ò?ï-–º}P?"úŠ"¼‹?šM(©vÄH?"úŠ"¼‹?ïÿË.^"'?ìvLA'}>úh´ÇtCÓ?ìvLA'}AGN3FGL J0533.2+4822@dE$û¨'@ rE AYÀ8uŸÕôÀ;<ERðgÝ?ë¨UTxÛ½@f»ŠPG@__áçç¿âå¬H·˜¢¿å±'ì>hW¿å•™(ýǎ¿çn[b¹fAGNfsrq@'ü£n/PowerLawTXS 0529+483?ïÿ2ØD?
W$‹,?]àÎó³•?
W$‹,?ﻩlÂ÷?Û09o¥?¹.Æ :?Û09o¥?ïÓ+̕"?lnp߅Èí?vj"ÂǓ?lnp߅Èí?ïìadª
?GðzÑÍQ?cžúÖo=É?GðzÑÍQ?ïýwËOo?4ÄGJñ?4A§§B'4?4ÄGJñ?îœõë&Ä?·ÐKÅA?¦0¦•ÅÅ?·ÐKÅA?ïiS­ÉsÉ?>½¼,?'ÕŠKøðÐ?>½¼,?ï¶ã$ʞ?sç(¸™Û§?'G6øöŸ?sç(¸™Û§AGN3FGL J0533.6-8323@r|˜`fÀ=&7PþÀ9Xå™LlÀÀ;š¬±¤RZ¿Ë,Ž@'á@æ±÷ßJ(@^*€J¿Øcî‡1¸	¿å\"åX<‹¿çåD¤Ž"¿Ó†fŸNí×AGNfsrq@µ ÝDPowerLawPKS 0541-834?ïþæÁPÓé?&BƒÅðs?!"êÜî1?&BƒÅðs?ïÏÌ°êz?'ûŸz™u?x§•—1?'ûŸz™u?蘿ŸŽ¿æ?'ÏÄ\–j?†ÛØP—?'ÏÄ\–j?ïÿ«f->óÔ6Þd£1?&uŽ\Ÿ>óÔ6Þd£1?ïü©.•>?BQ/&šÎ?:¶ŠbK¬?BQ/&šÎ?ïXÚîèDf?¨(¡<ƒÇ~?"ä¢$¯A4?¨(¡<ƒÇ~?ïÂë—?–]Ãg¡?½‡¸Û#3?–]Ãg¡?ïý‹>Íè?.
áhI]º?3§UfÖpT?.
áhI]ºAGN3FGL J0534.0+6759@bÄupÅ@22g  ‰xÀ9_UÅ.rÚÀ;¾ÜÛ7ɛ?ù¿y'3J°@`ñz¬¢?þµðØÜö¿ãY©Ìíƒü¿ÖºØª6Ûð¿àEåÝÙ©¿ë}™–ȦPSRPSR@•IÂ&€IPLExpCutoffPSR J0533+6759?Ô-z×·Œt?ÌÍôíïî?åéB"$9Æ?ÌÍôíïî?Î,ça§?ÇøñBøÎ?ètÆ'¹yÖ?ÇøñBøÎ?àûœÁAS\?¸N«øŒ$?ÞÆ}}YG?¸N«øŒ$?ÚÀãpÜ?¦±þæá‡*?⟿yŽG'?¦±þæá‡*?®Ãc)—E?µ;ƒÓ
ˆØ?îÉÈ$`K?µ;ƒÓ
ˆØ?µñFKÎ<?Àê>³Ö?íAÍöÿŒy?Àê>³Ö?É2Äý?°²µ¦=â|?é³{xNùÁ?°²µ¦=â|?¹k³Å§?š¾¯ˆZ'?ì҉ž5û?š¾¯ˆZ'MIXED3FGL J0534.5+2201s@g´ßݵÀö@8ªAÀ7®X¡UPÀ9×U,'?
?êy@wƒ3@dN>a@Ý_Ù.…¿ïÿô!O…ú?ïÒj WS¿Ùeށ*7¿ïø¢©Ô$OTHERPWN@Y3
å6PPowerLawCrab?ÒÌ%ëՄ4?Òpe*­1?æ™í
=æ?Òpe*­1?îà‡åşº?·•–C.ñ?¡÷¥]ÒV?·•–C.ñ?âŸÑøä5?³Pxô¤9?ÚÁè\7•?³Pxô¤9?ïÊ–kU¨?ƒ¦üû1?zû´Ò";Ô?ƒ¦üû1?åJ–Aº#?ÒgNJ]=À?ÕkþÓ|‹¹?ÒgNJ]=À?íwÞïl½v?ÀÄcšŒ¼D?´A"šO?ÀÄcšŒ¼D?çY?Ñ&N?µK# á:?ÑM€]³d?µK# á:?﻽Ë?"˗¦Kð?º°fù?"˗¦KðMIXED3FGL J0534.5+2201@g¨`ܹªÀ_?«'"À4V8/v~À9D›	Ü!Ô@‹u>›q@»7»ƒ#a@§FÀÙ¤w¿àï÷…nP¿ä'ÛÇ¿å5Ò$O•"¿êÆB9`sÞPSRPSR@ƒÜº'£SPLExpCutoffPSR J0534+2200?íF¤±í?Á©ð÷ö?µÊÚr;—?Á©ð÷ö?ÞHÅÎx?ú?×K'ŸMn?à۝Ãà?×K'ŸMn?â'ÃÑrñ1?µÅÇ,^^®?Úúx]Ÿ?µÅÇ,^^®?ãÞmÚÚ?ÁyÐTÛh`?ØC$ýæJL?ÁyÐTÛh`?ë_ãû?Ãå{©]uÁ?€sì—•?Ãå{©]uÁ?âÿþ@ÉZ
?×d;û¦!?Ú~mKæ?×d;û¦!?æ-'œÒß?¹d"êÍö?Ó¤úÆZAë?¹d"êÍö?èíO{é/"?Æt6j—šÞ?ÌJÂ[Að?Æt6j—šÞMIXED3FGL J0535.6-2749@lö²ßP]À;ëÃà•®À:oGÆ;À;ÇjM{³Ö¿æ®S+z)@
"½Y'B@Qç_u0"¿ê=:þèÜ¿æóh±´¿äÏ\wWØã¿ÖàüFYxAGNbcu@"'9Û"ÐåPowerLawPMN J0535-2751?ïý×Æ·?@Á>ÿ³aá?7ÉA»ü%?@Á>ÿ³aá?ïÔ³ˆO'°?…b๙?u¦;¼
\ ?…b๙?ï¼ëÛÛ³p?y&ƒ V?€Å		$?y&ƒ V?ïþÓÃiªF?h°s‹…é?"ÃÌ"?h°s‹…é?ï÷˜}dÚ ?V´·4Ç?PÏÿQ?V´·4Ç?ï8ۘŽùû?­ú5Y¶Ò%?˜äŒçAˆ°?­ú5Y¶Ò%?ïPø³…~?ŽH嗶úÚ?•àéŠ(Ր?ŽH嗶úÚ?ï꓎µ?_DJ›Naw?elq7»±.?_DJ›NawAGN3FGL J0537.4-5717@p˜Ô_õIÀ@6ä?°8À:q6Ô¨À;Ûµ_Ƚt?×35/s2@#)@oòä¼®¿ï¬qó''?å+ ¿þˆ1¿Ùé+(]þI¿ß#Ú½GÁAGNbll@¡lª=p£×PowerLawSUMSS J053748-571828?ïÿN¾Uð?hG_Åì?(97»4›?hG_Åì?ïÉ wP»Ò?'é!IÚG?{/Ä5õë_?'é!IÚG?ïæìË8½?mPè@ÁÊ9?iñn€²á?mPè@ÁÊ9?ïÒ«ÕA¡œ?[@ó¬W³?vªmÕ?[@ó¬W³?ïþ~e‹ ?'Ï'r¤£?(ªƒµ†?'Ï'r¤£?ï+ÃÖa©œ?§E=뫱µ?š‡….£b?§E=뫱µ?ïàǁ?so:¾I~³?oï8CÕ£#?so:¾I~³?îü§…ëfì?‹òÁ©BP? 5‡ mªE?‹òÁ©BPAGN3FGL J0538.4-3909@nŽ@îÙÀ>E`IôÀ:SÞKzQÖÀ;Þ|WisaÀf©!¡æD@¹'ùïÔ@S–‡å<¿é	ܘġ¿Õc)%úKÇ¿àðº¤ùk‰¿Ý1*Ê®å[AGNbcu@¥']Ùb·PowerLawNVSS J053810-390844?ïÿh5HŒ6?›°ð{?ùZeÿÞÎ?›°ð{?ïË=1¨ˆd?žŸO×|Ö?zag^vK?žŸO×|Ö?ïì>ϸS?T¬ÑcY?cèÁh¡DU?T¬ÑcY?ïÿÿZ]>›
°ýÉ?‹>"½HÞ%"%>›
°ýÉ?‹?ïÿ)V÷™»?OiTËe?Õ(ÿ›‰?OiTËe?ïFþ«N?¦ø'%€9™?— .ʖ<?¦ø'%€9™?ïäz¬!9>?q9¯	Ó?k…Sž.?q9¯	Ó?ïÿí )k3>è¢Í°Šß>âßÜqÃÊ>è¢Í°ŠßAGN3FGL J0538.8-4405@oB¨àÉÙÓÀ??Ï"èÀ5æZ¬ôÀ1À:Œáû2;?ùŸu‹ÈJ²@§9Bú?ÿ!L{ƒ®÷¿Û°.fçZ¿áÍ.õk¿á\"ÔvËu¿ã>oAGNBLL@|¬ÄLogParabolaPKS 0537-441?ïӄˆª!ì?…ÊwLJŸŽ?v=»¡P"$?…ÊwLJŸŽ?ïÆ¥‡IÇ?'k2ËPÃ3?|­<<ßíÛ?'k2ËPÃ3?ìN·Ðˆ»r?¯aó|?½ŠA{º$m?¯aó|?ïÿªõXÿm>ûB$!QÜ?B¹N"†²>ûB$!QÜ?ïâ "&Ø?w.ßËÞär?m_óÖ¨?w.ßËÞär?ï(,ìT?´6àŠñ?šúb{-?´6àŠñ?î9¾2ˆÆì?¢­ÄŠ8F¦?¬dÕ»ÃA?¢­ÄŠ8F¦?ïÿÕ¬Uš">÷8(œaÿw>õ)âAs%Þ>÷8(œaÿwAGN3FGL J0539.8+1434@gófŸê%À!B™`
Ü·À9Wßh°Ã'À;C2Öìá??ò8=-ÝÞÃ@Ìy³JDÈ@'(?7?Í02m¢à¿æ<¯ý»¾¿è­f}bT¿å«þ	rAGNfsrq@''ΊqÞjPowerLawTXS 0536+145?ïýÿ°W~Ë?2áʃóõC?0}	Ã~å?2áʃóõC?ï§ÀQ÷?"ÒõAdq?†뮯îT?"ÒõAdq?ï~ é?'¡ÐÕþ?ž;ýÖ0Ù?'¡ÐÕþ?ï÷–g¾ˆÅ?7|ï.FM@?PÓ0ݤ%±?7|ï.FM@?ïû·4Î؄?E'.yÜV*?A#-2°œ?E'.yÜV*?îTpêÅê?¶ž»ÒIQ?ª¸ñ_¿ˆ`?¶ž»ÒIQ?î¯XŒx? ådŽÃÿ?®n¥
í~? ådŽÃÿ?ïìglÿ:f?XÈåcPð#?c˜"#!±ð?XÈåcPð#AGN3FGL J0540.0-2837@mŸä6vÀ;@>€nOiÀ8ǵƒ+ßÀ;'j&ˆ?í…9Û÷j¹@Äo~)£@:Àß®¦Ç¿æë|ݘ™¿ëÇg©m³H¿çÔr¦™:¿ä½ÁA(AGNfsrq@wZYý6÷äPowerLawPKS 0537-286?ïÿr^õ·Z?öF¤y?´!ŋ­Y?öF¤y?ïÏ*Mí"ä?ŠSqM<w>?xjØøä?ŠSqM<w>?ïÉN©—yÀ?sñôëJ†?{X«,³ü?sñôëJ†?ïÙ#//›?S:´Ki'?snhFÈÜ?S:´Ki'?ïþÄ €Óû?*׫¸òh?#½ø9·n?*׫¸òh?îÔkåV[?´ÿ)wdéÎ?¢¹A®åÊä?´ÿ)wdéÎ?ï•çj4
?‡Š~[–!í?Š†›$(ì?‡Š~[–!í?ïEÇ:oE;?ƒÉ]³
à ?—G®§¼«?ƒÉ]³
à AGN3FGL J0540.3+2756e@f‡ÔŸ"…^¿÷þG€óšÀ7=ò¨(¨–À:"~áS?Òò"|/a©@{pkÍÙg@ŽHÀc1þ¿àÐÜ&$¿äŸ™±Ž¿ßÔ$"ï"¿ç †
 zOTHERSNR@†	©"áPowerLawS147?ì"o6?Ã[ÿôÜ$?¿{_$†OÃ?Ã[ÿôÜ$?ïx~KàS?¥™Khz?ý/¤½¢?¥™Khz?åPá(›Ìò?¸@j|ÿÊ?Õ^=®Èf?¸@j|ÿÊ?ïnF	­0ƒ?¢›w7k?'7>È¢!§?¢›w7k?êÇA…ää?·3üdr¤?Äñâùèln?·3üdr¤?ì/#ÿY?ÂÕÿ6½'ƒ?¿^†ç8?ÂÕÿ6½'ƒ?ç…PùåB?·8A‹¡Ås?Ðõ^5ÿ}?·8A‹¡Ås?ëñHäí¢R?ª$©'šÏz?À:ÜlIv¹?ª$©'šÏzAGN3FGL J0540.4+5823@c=éÀ"š_@,'‹ Z›À9P0uєÀ;€ÍÀÓg?øsÅ@~-'Š[¹@g  ‰x¿êoœß¹¿Ü÷&o!î4¿ÙÿhI¯:Z¿Ý}õ×KñAGNbll@¦Õ`ªdÃPowerLawGB6 J0540+5823?ïò4ò?Ue0ì?ZÅuº¤?Ue0ì?ï|6/Î
 ?s'ÇIG?y:R
?s'ÇIG?ï·2lõÝÎ?~íUïkç?'3d¿ðl?~íUïkç?îŸJÏþ?€9zûç[?¦_®·$?€9zûç[?ïÙs}"ð?pÀÝP‹²H?sFA%¹ËÝ?pÀÝP‹²H?êÇBì†?Ã9‹ ñq?ÄâôMç‹â?Ã9‹ ñq?îǪoeú—?£[ÎØ¡´?£…Y
ëً?£[ÎØ¡´?è´3g¥DŒ?­Ð"|Ñâ¶?Í/2ajíÎ?­Ð"|Ñâ¶AGN3FGL J0540.5-5416@p_öŸÏ=ÀÀ?ã^è¬À9%Fí$[)À;²u®ØÅÿ?èûµÈEËß@ žæµ,@ãßbüz¿æŽ‹î'¡}¿åឤJ¿ê<:áÛÛ;¿ïÿâÖEé¼AGNfsrq@{:Dg8~PowerLawPKS 0539-543?ïý‹ËG3?Jx>ýýK²?3{£<˜%=?Jx>ýýK²?ïÏÚÅw²®?‡t%PMsœ?x5¸M)?‡t%PMsœ?ï'ÔÊ?ß+¬#²~?‹ö
ÐìÖ¨?ß+¬#²~?ïæžq3»?MÜ…›>ñ?iaŽœW½k?MÜ…›>ñ?ïþ4¸»À,?7?Æ£?Æ!?,´qcPü'?7?Æ£?Æ!?ï=kÎã°ó?¬ä¼w|ÿ©?˜R† E´?¬ä¼w|ÿ©?ïl ~i=?úp½ó?'{ð/`<l?úp½ó?ÞêÓë?~kçÚ«?ŽÈVy?~kçÚ«AGN3FGL J0542.2-8737@rÅÈ _ñØÀ;Ð!`¢ØÀ:Þ$
%'À;·ª1—QÁ¿ò×øyùÁ"@LpjKM[@OÄÀ
÷¿ì|_ã{¡¿Å£/ð]¡¿Ê'Õލ¿çô%g~ÐAGNbcu@£‡éûçl‹PowerLawSUMSS J054923-874001?ïý4ZiqÍ?4¾µ²¸Ð?6]+†öo?4¾µ²¸Ð?ïÑ~Ý֊f?þz·Ìc?w@',é5?þz·Ìc?ïä8
…?i Rã_ˆ?kàìÂs?i Rã_ˆ?ïÿŽT…Ø>þÖ¨	ãÙ3?já⺫o>þÖ¨	ãÙ3?ïûÆöQ´?Dx1¦ÄÕj?@ä&'6*Ó?Dx1¦ÄÕj?ïJOJ|6C?¥ÅqÕ("?–¶®Ái¯?¥ÅqÕ("?ïÕ«ÿ*u¨?|W¬Üø?u*[¦ä?|W¬Üø?ïû`-½'"?>ˆ÷:Ç6?BJ.?>ˆ÷:Ç6AGN3FGL J0542.5-0907c@j¬ú D®†À3j矶êÀ9'ï,»À;
I"®P
?ð…««iûœ@£">‹«ð@Š1€€˜í¿æÌî¹9P¿ævx{Ö~ì¿é_}¹
Åx¿ïýÀ~FDAGNbcu@z¢!-w1PowerLawPMN J0542-0913)?ï+o´»*…?¢©mG¿?š'	fâáW?¢©mG¿?ìK{ï9´,?µêÒ
H?½¤ †2^¢?µêÒ
H?î/¦"Ÿ|?¦¾Þ1*?­%"VlE?¦¾Þ1*?ézOàÏr?š³Y¹M̹?ÊÀ|Æ8?š³Y¹M̹?ê¤+ÓîT1?ÅL'Y•XÓ?ÅoP°F¯<?ÅL'Y•XÓ?ÚåL²$?ёû¦‡œ?âuY¦íô?ёû¦‡œ?ælõE½?»9ò³ú+?Òß'Þt†?»9ò³ú+?Òr"ù]	Ø?ª¬o`S=?æƵƒQ{?ª¬o`S=MIXED3FGL J0543.9-5531@px+àXšÌÀ?z⟜èÙÀ8œûºöásÀ;bƒ'Öß?Æ{Jï<ŽQ@õ
j?üF·2»?ê¬ï^ñ¿ÕˆÔC¨e(¿Û̓݉w¿Í´˜õ&"AGNbll@©ReoPowerLaw1RXS J054357.3-553206?ïý¿›-dß?.RÎðð*?2%ÙîE[?.RÎðð*?ïÙY"¹›ö?~sI¨?sSn¤'Üï?~sI¨?ïӘñ'?vÖ
høTÏ?v3¹bY2ï?vÖ
høTÏ?ïø/3Îk?8VºÚN¾>?OC3Ù':Ó?8VºÚN¾>?ïüscá?A%Ûx•QŽ?<c˜6™á?A%Ûx•QŽ?ï4²n–z?°r!j|ÙA?™}é²-0²?°r!j|ÙA?ï½ð€Ü?"Q@
ÝöW?€ƒßËeš=?"Q@
ÝöW?ïÙ°PüX?gæ°âßQ?s'×w…#"?gæ°âßQAGN3FGL J0550.6-3217@m²€ÿÚ@SÀ:'q_¾¬yÀ:?¢óµnâÀ;›ÔÓ+‹Ÿ¿ä¶Î'¾À@
ØG)_J?ùÖg?Õ-¿èJÙºñØö¿ÕÓòr›x?Â_9è?U<¿à$ÿ³ÿÌTAGNbll@ºl¼¬1'PowerLawPKS 0548-322?ïÿE¹ƒÕô?þí9"L;?HÓd"RG?þí9"L;?ïÌ×xï¢\?‹ƒ²Û½?y"CšÉÑ?‹ƒ²Û½?ïå×ãßÁz?mé+͘4¤?j(6<&?mé+͘4¤?ïÿ}Zƒû?R/­,?T²î"¦_?R/­,?ïþÙnÿ? |ÈÂ(?"n5?°šä? |ÈÂ(?ïDÖ¼ÃGñ?ª]cBÑ~?—e(iNÏÑ?ª]cBÑ~?ïÞ­.̖?ye£jJC?p©iˆ'?ye£jJC?ïý³'=t?1t‹~O?2cnDèpÇ?1t‹~OAGN3FGL J0553.5-2036@l8rŸYÌûÀ5¢¡€èTÀ9¤i|›\À;‹"+ÁNê?ò"žÃO£@Œåõè¤ð?ÿÃA`r†…?ïßÉá']à¿ÒW—¡Fâ¿â:.³k¿çñ'‰ÿ?AGNbcu@žŒ"záG®PowerLawNVSS J055333-203417?ïŒaŠò?˜( n[9?Œçr<Ÿ?˜( n[9?íêñóDR7?±'À;fTë?°¨pd""Ë?±'À;fTë?îã²ò'œž?˜ª">Ö?¡ÄÐàë?˜ª">Ö?ëՀg"A?™¤VEÒ?À©ÿ¶a®ú?™¤VEÒ?í=ŸäÆ?¸(Û£¹´ë?¶à©N?¸(Û£¹´ë?æH7½¢?͈…¾#h?Óo'â"Þ»?͈…¾#h?çÚý¸¹*À?º½®D?ÐJŽª?º½®D?âø0V¸?²ÝØE5p#?ÚŸS܏Ò?²ÝØE5p#AGN3FGL J0554.1+3104@fc£ –x}@cý@,À8Çy*ŽIÀ;H5Ċß@ã®:»h@…'.¼!?ú[L¬Öã&?ïã'é9P?¿ß¾W˜\¤¿è¾ÈZÕ¿ïþÊ:Ì.ÂPSRPSR@©ë¹Œ~(PLExpCutoffLAT PSR J0554+3107?¶"Ü]'ë?—M·mêê?ïzKa8Q?—M·mêê?¤IÎ1$/ø?»f€xÇx5?î»cÒ@!?»f€xÇx5?ÀJ‰ßÍõ?¨Z¯ñIÝ?ëí] ƒ?¨Z¯ñIÝ?ªh'ue²·?åѾªô?îYwØ©¤Õ?åѾªô?¶Vì³a?…?[êq?ï¹Á&rÒÓ?…?[êq?‹ÓAR}?§íÚ;¾E?ï'²ú¶?§íÚ;¾E?»~€Ÿ³Ë/?°Aø]ÒÍ?ì/ì	†š?°Aø]ÒÍ?€žð5ԙ?oà+Ùù?ï½É"mã]?oà+ÙùPSR3FGL J0556.0-4353@oP`=WyÀ<®€±kGÀ9÷ªlO´sÀ;Ê/§î¿ÔaÀê–aV@'…€Þ@œ¸?wT¿Ä»Y¿±RÀ¿àšçg¿è•:í;Ø¿Ô|ÏMIx´AGNbll@˜ª—Oß;PowerLawSUMSS J055618-435146?ïûíJ,Q?EN¬Arš¤?@JØV·@ë?EN¬Arš¤?ïÌP§§B?'gÿ3J†ì?y׬¸o ?'gÿ3J†ì?cd?'¨q`sI?‹_g-'ü?'¨q`sI?ïüì=&É?%ã·Âõî?8ž<QŒ'?%ã·Âõî?ïî–XœyH?gá ³¦ ?ai§¢¿‡¾?gá ³¦ ?ï5Ð5ÚNã?¬·+nÜ?™EùFmñ¢?¬·+nÜ?îäŧóH?˜"5)í	9?¡³¥…n'?˜"5)í	9?ïÐ4'4ÎÇ?qÜAÉsÝå?wå·t¶ä@?qÜAÉsÝåAGN3FGL J0558.1-3838@n›Í߆ã´À:jÓ_ŽÀ9˜Q`Dä6À;–Å×Eî¿õq»v¹è@
ÞM'Ðÿ?ÿ]É^Ù)R?֋Áýïb,¿ç"	.Ia¿ÍîÉÄ&,‡¿Ú¯‰¿u»AGNbll@¥¥\ú¬ÚPowerLawEXO 0556.4-3838?ïýÉ81Ž‡?33JÂx?1¶=ýåóë?33JÂx?ï×C ™±?‹PïÆF×È?t^oΤPG?‹PïÆF×È?ïÌPÆʇ×?v—íš<Iº?yל­Iø?v—íš<Iº?ïÿ¹O'Á¡>õ ÞÜK?¬8›Ôè>õ ÞÜK?ïûKhR	?J)FV?BÒ`ÓèÇG?J)FV?ïOs£:Ø?©ð㥨ÜÞ?–‹œ˜õ?©ð㥨ÜÞ?í¾g?ˆþqõ¯Ô?‰ß—ET¿?ˆþqõ¯Ô?ïüÑÚ0?7Ò¤°wÇ?9wÍ¢?7Ò¤°wÇAGN3FGL J0558.6-7459@qáxÿûÎBÀ=‰ô?Ø]$À9´}C"À;¦üÙÚÒI?⦿aKÁÂ@A<4
Π@oß|&í?íh°HtÛ¿à2‹üU¯¿âda
~U"¿àoŸ"I<yAGNbll@ '§ï²-PowerLawPKS 0600-749?ïüø0—"?8/ÝL8%?8;÷"g%z?8/ÝL8%?ï³R'·è?RI»Ÿ?ƒ+[\ ?RI»Ÿ?ïÖ6x7O?rÔGÔKºr?täÃÓBÌr?rÔGÔKºr?ïfûñ—KO?t•$)«ü?" É¦ú?t•$)«ü?ïô"ïFÛm?Y3ù_ZŒ?VØ!S&¼?Y3ù_ZŒ?îÜ7Mõ?¸âÉƗ…l?®b<‡±þ?¸âÉƗ…l?ïs¸a/ð´?GG"ˆ/?'ˆóàá!†?GG"ˆ/?ì0Ñ
W?¦»-\u?¾Áw•I?¦»-\uAGN3FGL J0600.9-3943@nź@Ù$À:*Ÿd´µÀ9½
S¥™'À;zòÙ¦Ïã?É÷ù"•ø@g
}†@|­à#¿èHÛúDݳ¿ë»^säåY¿ëÖG¬*ڎ¿ïÿñY/WAGNfsrq@x´×6&-PowerLawPKS 0558-396?ïÕhåq´M?‡ì¨Ð½I?uK&م…?‡ì¨Ð½I?ï—Y"à'?˜îϙj?Š)šÎºó?˜îϙj?ïx{‰/¶?‡úTW`³ ?œð"s*?‡úTW`³ ?îÚ/úw2š?ƒ@ŒÈ‡ç?¢]ZD¤]?ƒ@ŒÈ‡ç?ïžH-Hì?——ñL(º™?ˆmô£v)a?——ñL(º™?êâ¥tU·?Ço¨9Dš9?Äuj/ž©#?Ço¨9Dš9?î1£H;z? ±¬•1Æp?¬æõÈ¬]? ±¬•1Æp?¡Ì…?·n3õôåû?Úüª¼gàö?·n3õôåûAGN3FGL J0601.0+3837@e§# –x}@"ÿŸÝÖ_À9ê+ùƒ=À;yóÐFÕ¿ÝÏàü7Q.@	9ùl?þ<ԟT±?²ût;Lm}¿än¯ñæ ¿ÆƄÜü£]¿àݺ¼$âAGNbll@µ'¯|í'hPowerLawB2 0557+38?ïþ˜ªíe/?"ã‹"$9¶?&uR-))'?"ã‹"$9¶?ï»îçÓ?"É/ìÿ2«?F)eÅ#?"É/ìÿ2«?ïÜèEÏ*?iœ2ƒ¾n™?q‹Ý$W?iœ2ƒ¾n™?ïúô(íp?1ÿ°:¢¼?Gœ.þÔß{?1ÿ°:¢¼?ïý'ÈŒB»?3¤8/ã)c?3q¼P	M?3¤8/ã)c?î¯ÌdQ8?µÈ]q½Î?¥>ø}?µÈ]q½Î?ïÄXº3\?€^M@b4??}Óþ¯ôÕú?€^M@b4??ïÏKŠíÚ?o¤Ï½Ííh?xrZ4YÆì?o¤Ï½ÍíhAGN3FGL J0601.2-7036@q­••À=Ÿ½@gÏÀ82ñc…
–À;]íCdٞ?ú#«kS51@º°Í@6ß"óŽ¿Ý-¯iBA¿æ!O$Í·%¿å0Ûrµˆ¿ç®(^P'AGNfsrq@N¡BoçLogParabolaPKS 0601-70?ïü	õ»ó%?<"<
†n'??°Qb/¯š?<"<
†n'?ïÉçE°§?‹KÞ@`Äñ?{]G?‹KÞ@`Äñ?ï>¬Ö?ï?"Œ×äKý?˜*e3l?"Œ×äKý?ïë/ʘ?NNM|éÌ?dÐàRD¬<?NNM|éÌ?ïôIÐ|Q?[(–™Ù^A?Wl_[Ӎù?[(–™Ù^A?ïõÁýTÄ?±ðcðÓ-?AGÅ|с?±ðcðÓ-?ïLmŠƒ7i?"ôrxR?–rN±Pàç?"ôrxR?ïßô˜ {?eò-MÐÌ@?px…•F?eò-MÐÌ@AGN3FGL J0602.2+5314@d~`Ï6@-,}C"À9Ñêä±À;£¾:bÒ]À©ƒæTi@«¼pP±@Du߀-¸¿í'>9²ºc¿Ã¬Ò['¿Ø ÈýµLþ¿á<$§cvAGNbcu@¨W^šPowerLawGB6 J0601+5315?ïÿ!åvÅ?µ*r¿;?ÜEòS?µ*r¿;?ïØdë™y?"`N*w¦>?s͊p´ƒ?"`N*w¦>?ïéàCw#"?c*ß?f¼Â–M—?c*ß?ïÿüè‹+>´WbtÒm>¸¿hªÜ°>´WbtÒm?ïþÀ"ç®?'&zCÝW†?.´þ>ÎW?'&zCÝW†?ï'|tï…?°ý'g{LB?›|tÑ«\?°ý'g{LB?ïä<þ8)½?róI¾h?kÃ/ڟ?róI¾h?ïÿ¸{ Ï?Ûº
™²<?á²wM?Ûº
™²<AGN3FGL J0602.8-4016@nÜ"ÿ‰;À9ó¡_`¸§À9#¾ôœõoÀ;V»ºUÑÄ?ä¾*ós«@=
¬æÓ^?þÄ6á=¿´
'½'¥½¿ÝyKyÓÍ¿Ê¿±})æ¿ã±þG÷™AGNbcu@§ù•Y³Ð}PowerLawSUMSS J060251-401845?ï÷D͉®?QÖÿÜÎ@?QwØÅ!´e?QÖÿÜÎ@?ï´DÁ-º×?‰ªáîñ5?'îϨâžY?‰ªáîñ5?ï¾5U"…?6'2s¿p?€rœ·Q¬˜?6'2s¿p?ïVÕ5Y²?qBNÕã8?•/ÅaëÏ¿?qBNÕã8?ïàθp…Š?kì¨D9Ã?o1G~üUÃ?kì¨D9Ã?îՎߣ¶?¶)¬ê‹"?¯¢§rœ?¶)¬ê‹"?¾¦ì?ŠÇÙ֝?ŠSP][<÷?ŠÇÙ֝?í-™¼¡~?ŸÏčˆö&?¶—S3dΏ?ŸÏčˆö&AGN3FGL J0603.8+2155@g"	Å!Þ?s\žà*­À9dûy‰À:þËåF@V¿þ€v²äÄ:@ɦ$Š±@βÿœ,ò¿Ý±ÙH}"£¿åö>
3¿áª<Üv°X¿ÚõÓS'pAGNbcu@­³üj~ùÛPowerLaw4C +22.12?ïÿÅIÃ>ûÆh¬•">ý[%Ѫ!>ûÆh¬•"?ï¾þÝ/	r?‹™~îQêŸ?€@H¦3¦?‹™~îQêŸ?ïÃyä	?ƒ
?>oT‰?~|Âôˆß×?ƒ
?>oT‰?ïÿÿ…—ë*>"júϾ¹>Ž£L4'Ý>"júϾ¹?ïÿˆakˆm?¡ñ0p?
矄!lY?¡ñ0p?î1ž[}ݯ?ºàêÕ»"?¬æFjW?ºàêÕ»"?`I…Ÿ?ÊÆË•ß?'ñ4F?ÊÆË•ß?ïÿúœÇT>ÊÃ%Ïd>ŌØ­¡>ÊÃ%ÏdAGN3FGL J0604.1-4817@oö:à;>šÀ;€¦@q	XÀ:O
ª}ílÀ;¤Wèõ!€¿€‹G†¦F¬@5~ßÙïË?÷J` |!¿ï½Þÿ¦L?ïCy^]$ì?áMó½ÉÇ?˜–Œ°¹,AGNbll@ÇØͲ-VPowerLaw1ES 0602-482?ïþ=N®Ó?-léH"ªƒ?,+5l¥›?-léH"ªƒ?ïÔ§#gZ¥?ŒÚif¢«¤?u¬n,¶Eè?ŒÚif¢«¤?ï§@n¸'?‹k3p>N?†/ùdQی?‹k3p>N?ïþî•Ìt?d.Y|¤Ü?!EË£s?d.Y|¤Ü?ïþ?–)3?0QîFtêå?/¬ÿº/?0QîFtêå?ï<˜Ÿ•?«®`•µí	?˜lý
]?«®`•µí	?ï̍SSþÊ?ÉÌ&³˜?y¹V\ßÓ/?ÉÌ&³˜?ïþ‰kVú?$p¨¬›ë!?'iJ{"ñÚ?$p¨¬›ë!AGN3FGL J0604.7-4849@pã_€™À;€¹ Gž$À:T>iƒQÀ;ÅûqûÅß?¶Pf"ÀŽ@×_´Æq@0bŸ²bh¿á7ÈK]Ìd¿í|jŽ‹•í¿~ŒË*
j'¿é܈¬ŒeAGNbcu@"Á§†Â'PowerLaw1RXS J060432.7-485007?ïüß?Õ²??m—Ãï'?9HˆG??m—Ãï'?ïÄùS_ðÎ?‹kඪÆ?}ƒVEÙ%?‹kඪÆ?ﶨç
µ?€f	ÎM¾ï?'UÆ25Pª?€f	ÎM¾ï?ïÖE'Âv?a<3ÜT?ú?tÝ6¿Á3Ú?a<3ÜT?ú?ïøµî[_D?TèÞÿëåA?M(Feû4Ê?TèÞÿëåA?î®üú‰jð?µ¸(ՓA?¥0Vj?µ¸(ՓA?ï*ðOø?'m=-"œ?š¡öv]?'m=-"œ?ï	Qf¾¿³?—!ë"÷q?žÕÓ((	¬?—!ë"÷qAGN3FGL J0605.0+3756@eƪŽ:Á@ü.ŸûˆwÀ9³¤™_¸À;®yð'Î?û¾æ‡^@
|€È'Uƒ?ðü—x,6•?ïõ»tpüS¿ÔÙ3î"¼¿åª§Ç|¿ïp<"
œ(PSRPSR@˜ÔɅðoPLExpCutoffPSR J0605+3757?pý)͋?u¹æ$fƒ™?ïÞ¬'D¼?u¹æ$fƒ™?°ø¤Üú´•?ÃayíÎ?íàëd‰ä½?ÃayíÎ?ÁE"Hµ¸?­€ÈÞC?뮜žíҒ?­€ÈÞC?¹ùz'?™U33F·?ìÀм_[?™U33F·?^Úe؜?X	\Eaœ?ïð'óžY?X	\Eaœ?"Òn¿Xù?ªöLöCaÖ?ïao<Š8?ªöLöCaÖ? ‹¡je§ä?•¦	¿qo"?î÷E鐟A?•¦	¿qo"?‡SY½bUó?t}Wÿ?™3±ø?t}WÿPSR3FGL J0606.4-4729@oܱßv½À:÷ûÀÖ…À:üLû[À;ƐY~÷W?Çû¿¥-1Î@Ë|½ë³m@žšÀ
F«¿ìœ­¹rc0¿¹"¢L×°<¿çöK¨ÂMå¿Úq84'q=AGNbcu@•¢$?åÉPowerLawESO 254- G 017?ï÷ž¾°2?[Âú¨Lñ?PÃÆÇWËw?[Âú¨Lñ?ïÈþ&"œã?Š¡ŸÜۋø?{€ì¤J‹?Š¡ŸÜۋø?ïus½?ƒâE(ë?'Qˆd¼7ì?ƒâE(ë?ï·ÉV0õR?gÄp7k–B?'
ªx'–?gÄp7k–B?戀WÑx-?ë·™jçÙ?†[éýã"Å?ë·™jçÙ?îU"áP½?±Õ¡ÎF?ª®g°3&-?±Õ¡ÎF?í¬#ƒw?¤ÿ#'$†ý?²žç?ýJ?¤ÿ#'$†ý?ë屎òp?¯q=g¼?Ài9Ä5¾B?¯q=g¼AGN3FGL J0607.4+4739@d´xÀ>-@)ºžEÑÀ8E&s1PÀ;?uQ»´wÀ¥Ç¥EŸG@[sºÿé@.>`7ù¿äåÉkvú¿à\¬‡n/¿ßs"¦1Fc¿äª¯¶¼j)AGNbll@Y>ߤ?æPowerLawTXS 0603+476?ïü¶h§£?01ºJ©ë›?:L¾xs…K?01ºJ©ë›?ï؎YþÕ?}¦<'£Ç
?s¸ÓíQl?}¦<'£Ç
?ï·N«šß?…±@âð»ï?'8¬`Çô&?…±@âð»ï?ïÿü&NØ>ÈUœjÒT>¾Ë‹¥MØ>ÈUœjÒT?ïõSËrôX?Qxüs·?UXh˜æ~?Qxüs·?ï>éË=ß? 3
Øœ?˜"Ɲk‡Ï? 3
Øœ?ïUvq¡Wÿ?"ccw°"?•Q1ÄõÈ,?"ccw°"?ïÿt=OÒâ?dazͺ?xQæüêS?dazͺAGN3FGL J0608.0-0835@jø€àe0À+>~ÀÐ?À8VÆ;¹²À;£NNA¬?äQ·
%‹@i°Ü+dˆ@û>_a9¿ÞÈc¬!Üt¿æêðü××m¿äŒñÍ'¿çŸ°·ìÏAGNfsrq@†öŽAcPowerLawPKS 0605-08?ïÿ;œ…ª?W[§Ñ·?X"Sj3?W[§Ñ·?ï½Vlj®Â?ŒFW@Ž?€ªdÞ!?ŒFW@Ž?ïÓüá‰êœ?pô‰¡Ä$?vNøm³?pô‰¡Ä$?ïõú:Ä!?9v¹
7?Uö$ÃN4?9v¹
7?ïýú"k	8?1IþfÓt?0+Ýåx–?1IþfÓt?î[S
Å^?¸Žåä}¼?ªJÐx?¸Žåä}¼?ï-4"Ó3?'Ì$šäÔH?šYojè?'Ì$šäÔH?ïÕ¨JƒÔ-?d<Ä>s"?u+Ú¢™	¶?d<Ä>s"AGN3FGL J0608.1-1522@kÄUŸnÅ°À0cZ _†xÀ8'™" äÀ;`l,yÏ?÷•<ÀO»Õ@O?'¡Û]@‡Xöç(¿â=³œÐæ¿ç±ë~$|¿ê±¥?s¿èKÎxژyAGNfsrq@t	¦">jLogParabolaPMN J0608-1520@?ïýX'¢»h?>'SçÄ?5;r0S~m?>'SçÄ?肋ÝíÜg?›S¶û)?†›vÊvV?›S¶û)?¿°U?@#fûw[?‡l†¦?@#fûw[?ïzoª²Æ'?p¹íh£?²
§ï_Ù?p¹íh£?ïó×ÇÁcý?VJ~Z?XPpÝmô?VJ~Z?íÍ(êQdn?½G{K.Ç?±–¸­tܐ?½G{K.Ç?ïd#Nl?¶þâÒ%Z?"{–@¢C?¶þâÒ%Z?îÄæpÚ*? ÿ4.?®±™ÎD]? ÿ4.AGN3FGL J0609.3+2131@g£? §??íÀ &jgÀ8Ӟ÷§kêÀ:Ý12I(?ýSj-E]'@
géÝSؚ?ûè!¼é*¿àñqÇÿàå»,]¿ìK¤™'¿ëz¡5¼œËPSRpsr@"y=ÙLogParabolaPSR J0609+2130?Š‰Gó
?šî•r¹'?ï•ÛÓ;"?šî•r¹'?¬d}^ù«??ÂHò½®?î9¸)ôèl?ÂHò½®?ÓALôØã?µŽL?Är?æ_Y…"Žy?µŽL?Är?¶Mƈ­;¢?"X•PÁ?í6G/"Ü?"X•PÁ?Q×$1,?LÛr/ª+G?ï÷nƒÒ?LÛr/ª+G?‹1&aÀCº?¦Û_ÓÍ?ï";f]'?¦Û_ÓÍ?¦¶$ö¡¶?Ÿfžcš®?ç¤?Ÿfžcš®?|"r•I)÷?k[½7"ìí?ïÆÙf,?k[½7"ìíPSR3FGL J0609.4-0248@jT&Þüz:À%AŒ 4RîÀ96ÕVß	æÀ;:"Ž½ž?Ñr†]…Iß@M>A©™?þ_O€ñ­¿àWƒ@€'{¿Ý¬)AusÓ¿ÝÙ«‰þhs¿×À›
–AGNbll@®Í4êJŒPowerLawNVSS J060915-024754?ïý*JX…?-ë+ºÛÿ›?6­ª®­ÅX?-ë+ºÛÿ›?ïºÎ'A-?Žl¦g"V?L[}Ë!?Žl¦g"V?ïܗÚkŠ¬?l(!+{³E?q´ÙXñ¾?l(!+{³E?ïï{•o	ð?Bv "›?`"jÃÐGS?Bv "›?ïô4-À=Ù?Tk©:±4Ë?W—¤@K}?Tk©:±4Ë?îOývìN?»šʋÔà?¯;(';?»šʋÔà?ïŽMÞã®C?‹APkù?ŒlˆGo+?‹APkù?ï‰F·G*?y¨°/T£¾?®z՝љ?y¨°/T£¾AGN3FGL J0610.2-2059@lwXf€À2-ПÀ$HÀ90¾£%4À;	Ü!Ôf?óûíÖ]@q-­ã(@°}_|<g¿ày·ÜBx¿âB¨ïM¿èvN—×fs¿ìŒ»[•ÄPSRPSR@Š˜r䎊rPowerLawPSR J0610-2100?¿nÃÏo‹Ë?Àé
M¿Y$?ì'†‡?Àé
M¿Y$?ÁŠ,<&ªl?ÇÙ¸ktuÑ?ëtðöUe?ÇÙ¸ktuÑ?å0®£?²…ـÒ?Ôáñžà¢º?²…ـÒ?η#Ã(´)?£‰àu?èR75Òö?£‰àu?|bD°âë?†U4êâDU?ïÇ;vßÁ'?†U4êâDU?¢3*íÇ÷¯?¶kZ'O
?îÜÍQh8µ?¶kZ'O
?ÉÐÁùà[?±ÓƒÛæFü?é‹Ï‡ÿé?±ÓƒÛæFü?'œ;ýŠ™q?zk×(ð3?ïkêoå?zk×(ð3MIXED3FGL J0610.6+1728@h" ³Ô®¿èbšë±À8ÓÿgSÌ0À:ò+ÐÂü?üEy Ó4E@Êê?«ç?þ,Mìm¿ÏnA§V¿è神ç3¿ëؒ2>¿ãl¾U¼OTHERspp@Œ:QN;Í6LogParabola?è4ªè)'I?̈́¶í<?Ï-T_[bÛ?̈́¶í<?Èv'`²?Èt`U'h.?éúâxŸgÔ?Èt`U'h.?æö¸ªÅª³?µPü×2€?ÒŽªtª™?µPü×2€?Ú.ºtýÐ?±"BŸ1À	?âüh¢Å?±"BŸ1À	?Ú47ÃCiÀ?ÐÔî%ÚR?âåä^K ?ÐÔî%ÚR?œ=JºîÝ?¯qÕaD3N?ïª6Ié?¯qÕaD3N?åÆpè?¹pDÁÞù?ÕØs/Àã?¹pDÁÞù?²+E<Wñš?¦ûÄEº€a?íº—XKÆ}?¦ûÄEº€aMIXED3FGL J0611.1-6100@pá´™=SÀ<O <¶jÀ9‹€ì#ªÀ;Ó\9¼º0¿þÝ3Tk<9@ˆy½0M@£Z?¼ƒ~¿é\ºO5Œ¿æ¸Á¤>}¿é`Osä0õ¿Ú•"»T7AGNfsrq@{‹úÁҝÇPowerLawPKS 0609-609?ïÿ¢Iì]6?
/*�myUK+?
/*é¨?ïÛ'º?g°?€"!uö›5?rl"ÿèÂ?€"!uö›5?ïÞ¤>c=?h†zÐ¥"P?pû­ñüm`?h†zÐ¥"P?ïÿüzŽä>ºt'E|{!>¼.É®Pi>ºt'E|{!?ïþàõgu?*=¡¤+ž?!ð­"ùQ?*=¡¤+ž?ï7Þw*j?°	¿÷S¸?™1jŠ\?°	¿÷S¸?ïÊSâ;…"?yMʂ×uœ?zÖúJ²¡?yMʂ×uœ?ïÿ–|ó_w?B[ÛöÔ,?
`ƌNÆ?B[ÛöÔ,AGN3FGL J0611.2+4323@e;R`õä@' ^YQ«À9Þî<³åÀ;¤ÏFúT?ÕL¯/æ)@´8V]°@Wé`}¿ë—&Z1ϱ¿ãn"±Ž"¿×'Œv4S‰¿Ø`|ˆAGNbcu@¡ŒR䎊rPowerLawNVSS J061107+432404?ïþ,uvF%?1ãb®?-8¦s©C-?1ãb®?ïÄÅyÇAH?ˆ·N·þFˆ?}CPØC?ˆ·N·þFˆ?ïä<ïŽ?pN†Žå?k~úþ)¹Q?pN†Žå?ïÛ¸ªx[~?S^nô'¬?r#ª©M??S^nô'¬?ïúZö+üï?G©©À_µ?F"&bíú?G©©À_µ?î†?"oi?±v™TôOÓ?§œ
á@×t?±v™TôOÓ?ïÑ¡—Ž
?~–Ü'H¼?w/w"œ'¿?~–Ü'H¼?îá/j ??1V)Ña?¡íh{þú??1V)ÑaAGN3FGL J0611.7+2759@fõ¢Àh¡@ã:"À9«œàuöýÀ;Då1?†sðº±@.Ääv@7¹½ûN¿åÓx³£Ž™¿Ûõ>ŽŽ¬¿àÞꌃå¿îŽ'ÞQQAGNbcu@˜¶/Ÿ¾wPowerLawGB6 J0611+2803?í,Yy1Þä?°ìGàÙ
?¶45•!á?°ìGàÙ
?ï´Èð°gø?'ìEöÊÆ9?'ÍÃÓæã?'ìEöÊÆ9?é§Ðq!õ?®ÎylŸÝÎ?É`¾;x.?®ÎylŸÝÎ?ïѵNxUt?Zû|?C]?w%X¥˜¶\?Zû|?C]?é­MmŸ?ÀQe©ƒ?ÉKÆÊKµ'?ÀQe©ƒ?îAq_œPa?²}&yïã±?«èêàò?²}&yïã±?åæýˆÒ?·˜2b|¿?Ô3îÎî]?·˜2b|¿?î]ì
eñ?—ŒŸ(‡…?ª.!AíUñ?—ŒŸ(‡…AGN3FGL J0612.8+4122@ezWà&Eå@%Ö3À7²8%
{"À:à"Xð\?çXwýVq@@¡)3!@3å?ŠY‹¿ÙíÕǃrø¿àïr«20¿à6tJ¢¿Þ5	cÎSAGNbll@"ŸÎV"PowerLawB3 0609+413?ïÿœñùé!?èMaÙ4?ÅÊK?èMaÙ4?ᅢi2Û?‰l:zu?€8ri×C?‰l:zu?ïØú
ˆåÓ?zzê4šD?s'ùYº"?zzê4šD?ﶌœ¹';?eÏ÷%p9ê?'\ØØ"³5?eÏ÷%p9ê?ïþ—AœúÄ?*ïrÐrª?&‹ã}Õo^?*ïrÐrª?îz9©2؉?²äÖš£?¨\eof,i?²äÖš£?ïºI¤'«Ú?Š­~dB?m—s¡Z?Š­~dB?î€!wbÑË?–ºÄ¡*À?§ýè‡?.Q?–ºÄ¡*ÀAGN3FGL J0613.8-0201@jMõ¡lèÀ"—ô|ôÀ8
¤ž°ZÀ;#wÀOç@ÿ…$'@<ó%|?þ5لÁ¿¶CÛ2Qr¿ÜÜ#€Òg/¿ä°·•­ü¨¿ïJÑz kPSRPSR@ƒd¨ÁTÊPLExpCutoffPSR J0613-0200?C"pæ1
2??ãbW@¦?ïû7c™'s??ãbW@¦?ž …}=ò?´]*¯U?ï
ûÓíÊÁ?´]*¯U? §Ñ!½Œ_?–=ùÒlÌ?îõ'î(ßj?–=ùÒlÌ?Šï­L~Þ­?qÄ
-^‹½?ï"AJÎ…?qÄ
-^‹½?IQ¥£r"í?D"Û"V?ïù«–W?D"Û"V?¤õ¤N¬Ë?¬I™µû¯?ï‰l)7ˍ?¬I™µû¯?"
·u8?~ä÷ʪO?ï­¿ÉY$ß?~ä÷ʪO?` ¶dC·?R½9)iøA?ïïßIYÃÉ?R½9)iøAPSR3FGL J0614.1-3329@nà`þG™À5Ô´ßp=€À6ì^'À:œÆä@ý#¬¦@u˜>¥­#?þÞt§Ç¯­¿À'ª~nE¿Ö…¦|X¿áXez`Í¿êz¨Ea'žPSRPSR@‹r
ÀƒoPLExpCutoffPSR J0614-3329?»Î¨1F?§èùÎï"
?œ#ë?§èùÎï"
?±ÇDñ5\º?Å(ÀYˆÍ?íÇb¹?Å(ÀYˆÍ?ÇŽÞ§«?°ó`Lî[˜?ê<H`?°ó`Lî[˜?QK7LL¨³?@¨µß=?ï÷Zd´?@¨µß=?—™E#BÙ?¶",6Ö$?ïC5×ש?¶",6Ö$?›ì1Ì=Ì7?´‰dTSÄl?ï žq«Ð?´‰dTSÄl?®'Ãvî¼?¤;Hºàº`?îÓȃUÏ?¤;Hºàº`?)ý¶>ÑG"?(æ!ø+?ïþ`$¥HF?(æ!ø+PSR3FGL J0615.4-3116@mÊòŸYÌûÀ4ՙÀ0XÀ9Òâ7˜ÂÀ;ÇyÒ9À'«0ð¸º@:ÀÌäIÁ@¥@¿ ¿é_äy'¼V¿å…Â+¼¥¿á"",zåØ¿á¸]Üv…eAGNbll@¹Ë)^žPowerLawPKS 0613-312?ïþçµ×?+܆T@®?!"±ÕÁß?+܆T@®?ïÃo3¨©?"×ùëWÁ!?~Hfnœ‡_?"×ùëWÁ!?ïëç^•Ùé?b9Vv ô?d¡:a?b9Vv ô?ïÿü†g§s>ºü¤ÿ(È«>»Ëèàƒo¤>ºü¤ÿ(È«?ïþ)ûjÞµ?0Kmq/½?-`F썧?0Kmq/½?ïE+'²ä?©ús÷d9?—Z¤•yŽ?©ús÷d9?ïÌYØÂ?xí]^}€^?yÓŒqŒc?xí]^}€^?ïÿ Si€ï?
­BêlB'?ë0´eû?
­BêlB'AGN3FGL J0617.2+5701@c­UàqÅ?@2ì_9K{À90½7-"À;"*m'ÓÒ¿úSndzÞ>@OYãÌÆ@T?b¿ÜsOa«ÛT¿ä1T>y@¿Û©NßG^õ¿ÙÛË}lg\AGNbll@™åSt¼jPowerLaw87GB 061258.1+570222?ïþ/Å.a¬?"w©ö	,?-«IæÎì?"w©ö	,?ïÖþÔÜ»­?…?þj '?t€•®~á8?…?þj '?ïá饱¼?m?C̶?nZHĔ˜?m?C̶?ïÿðd›Nê>Õáö˜yu>ß6GŽOB>Õáö˜yu?ïýƒ°=
ì?.–Nì/?3â~z…]r?.–Nì/?ïGý¼ü?±•:M'Û?—AE3?±•:M'Û?ï¾Aƒ€å?'hv+kkÆ?€oºÜ Ú?'hv+kkÆ?ïþÈ*O?&;U…§?#ǁw!"6?&;U…§AGN3FGL J0617.2+2234e@g¡ŠŸb0@E?ªºÔÀ5iL"=À9¯Õh|Á@M1;ŒH"@d³kýª?ûwohÁh¿ÏDô¦°ƒk¿á4U݂&¶¿áW35å?¿ä鯁7xOTHERSNR@–àù	kºLogParabolaIC 443?Üð&óM®Î?Öq¨¶k?á‡ì†Y(™?Öq¨¶k?£kL=ëÿà?¿húÈç?îÉK<X9Â?¿húÈç?Òª˜â[÷š?³oQxkí?檳ŽÒ3?³oQxkí?v8Q/?eq™¡¯n?ïӎßùœ±?eq™¡¯n?Ñ^z<d½Í?ÓxµB±ß?çPÂáÍ¡?ÓxµB±ß?ŠÛ_h™'%?ªØ[pE
Â?'4^h?ªØ[pE
Â?à=("Ḇ?¹-ŒN?߅®Ø<Žô?¹-ŒN?OŸÏó¦Ù&?LÈ»Áý?ïøŽ?LÈ»ÁýMIXED3FGL J0617.6-1717@l¨ŸÆÚEÀ.1Ïþ°t§À92éf`‡)À;PñîÅE¿ç`Úö±!Ì@­À'U'z?þú¤¾æ°#¿ä6À'«ZP¿àb
¥^ó¿Úmœ;èí¿Ï¥{ÔP"…AGNbll@¥Á:'£PowerLawCRATES J061733.67-171522.8?ïË[kǵ?³kFÚÎÐÛ?zqR?ÍQU?³kFÚÎÐÛ?ïÂ'uöã]?³%<ퟕ?~ìDöõ?³%<ퟕ?ïç^K9å)?rýö¤Iê?h¡´þtn£?rýö¤Iê?ïÿ¨ Xáª>ú¹°•;û?×é-§^>ú¹°•;û?ïýÓ2 í?8îÈJ¾?1fl݂3m?8îÈJ¾?î›è'ÇN?¶ށÿ?¦A~Æ÷¤&?¶ށÿ?ïß–
Ìj?xAª>ü?p5§²?xAª>ü?ïüÃïûÈZ?3sLM¬?9à~áÇö?3sLM¬AGN3FGL J0618.0+7819@`õÖàL'@8Üz¿¹¾ÓÀ:ZÍcˁsÀ<ÿ¼ä?娖×@Âùó÷^@ùÏãJ=¿çÖý3¿éMb˜óμ¿Ú¨O‹1U¿â/p¹"#AGNfsrq@'ÁA [ÀPowerLaw1REX J061757+7816.1?ïÿ€ ›¸Ð?'"€
§?×àn̯ó?'"€
§?ïÂ;Ÿpü ?†6JنÞE?~â0'5\,?†6JنÞE?ï݉DÈî?v I?qt;cÊÔ÷?v I?ïHc,[d?k@ãgžjÔ?‹íç4é'?k@ãgžjÔ?ïÿ'L:Ž?ÍQ±Ñïì?­Þ‹ÃBŒ?ÍQ±Ñïì?íœu	Óy ?¹ç×j4§?³W²@ü?¹ç×j4§?ïŽÝ)4­?†»GË7ú­?ŒH¾¼'Ê?†»GË7ú­?ío*ÐÁ?¢ÞTH>¤?·4†ªµ'ø?¢ÞTH>¤AGN3FGL J0618.2-2429@lü1 žÛùÀ1Ï~¶ß%À:›¹.ŠWÀ;ÆĹØÔB?é4Ê]9tž@Ì9¶3k@U'1>¿ß¹Xôk—¿çöçMµ6¿ägÄäÝ¿ïÿ´ó‰œnAGNbcu@‰‹8þï^ÈPowerLawPMN J0618-2426?ïÏw*ȚR?'b;sÜ?xDj•ƒ‹?'b;sÜ?ã4]{ln$?ÊþݯâË?ٗE	'#¹?ÊþݯâË?î"ü"±'?šò0evÇö?­ß:H›è?šò0evÇö?å
ʸ4‡?¦ îëŽ6˜?Õêkʏ–ó?¦ îëŽ6˜?ïO&ÛOá.?¦'S²¸,4?–$"LO?¦'S²¸,4?À?ÒËÇó?ÄÆ¢ñÜü›?ëð?KM?ÄÆ¢ñÜü›?ì-?ð99?©·í‰ß&?¾–N6;?©·í‰ß&?¾O½`%ã?¡íÎü²*¦?ì6SûCœ?¡íÎü²*¦MIXED3FGL J0618.9-1138@ky /µÐÀ(Ø´¡\ÜzÀ9•o"'ßÀ;LžáØÀ¤ê…š^@	Ýr"rl@ÁƒÿÔa¿ç8¨¢˜h9¿åjŽ‡[˜¿çMû¹§ß‹¿ç2uâ@ AGNbcu@‰UˆÎp:ûPowerLawTXS 0616-116?ï vâ×È?¾ÞH,6L?›þ#¥ñ?¾ÞH,6L?ïÄñh¯ä+?'qJÓµ_£?}‡K¬Ý^a?'qJÓµ_£?î¥Ylò‹g?žýÆâ?¥ªi/ûb?žýÆâ?ïÿí¯žŒ>ï¶ÀÏf']>âP¤w¾µç>ï¶ÀÏf']?ï'n7@3?'ăod%"?‹»är/ó8?'ăod%"?îÎ=テ"?°a$¨é´?£!;æä?°a$¨é´?잝:®?©زeÏ?»/R*?©زeÏ?ïúa×¥1Â?P[ªá1â?Fx¡:غ?P[ªá1âAGN3FGL J0620.4+2644@g6§?tŠ@‡'ŸÐ€À:F…íë*†À;ƒÜÌõ¹?Òi)ðûfy@µfEjC?úfz€NÄß¿ïÿüØ`?ïÿ›ß*ž¿×b÷ÌT×É¿àîúz¿	AGNbcu@ÁM8Ôýó¶PowerLawRX J0620.6+2644?ïþÁcâþg?!fùy7J?#é¾Û¢¿µ?!fùy7J?ï‹!Ó~0¡?™:lÄk­¸?7‹%»?™:lÄk­¸?ïÖíb¢E?ní_üP¼?t‰NŒ™Å¨?ní_üP¼?ïtMC:ù?xÈ¥<e1?'ÖW˜ Ô?xÈ¥<e1?ïûŒDé¶_?Aô¸èÙ¹?AÎíë¬æ?Aô¸èÙ¹?윱ùóÞ?À¹e
ŠŒO?»Zp0a?À¹e
ŠŒO?ïÀ€°€}?}ÍâDWñ¢?¿¨?!¢?}ÍâDWñ¢?ì..
{àî?ªëò¹½ÈÅ?¾Ž" ø?ªëò¹½ÈÅAGN3FGL J0621.0+2514@gcRàãG@;îN.ŒÀ9:ÛWªÀ;:‹#µî?ôø / V¢@6|CG}m@],¿ü"Ë?﵂·ï‰Õ¿ãèðjwµ¿Ý4À£ý¿îÜy'Š~PSRPSR@šåš…‡"ÞPowerLawPSR J0621+2514?Ö›¾s(þ?ɦ™¼ÝŸ?äó² Æk?ɦ™¼ÝŸ?Ƌ¢#DÂ?ÇàŸ °é[?ê]<w.Ï?ÇàŸ °é[?â,9öµ˜B?´Ÿú0p%Ñ?Û§Œ"Ï}?´Ÿú0p%Ñ?Üïî	v]?°Mí+ü'ÿ?áˆÿûDÒ?°Mí+ü'ÿ?­ºé¡Id?²TÚ9"Bº?î$Qeù.*?²TÚ9"Bº?°P9ÐY"ß?·«-"Œ[?íõøÆ‹Ô?·«-"Œ[?Â1 ѓ"?¯3‰âoàÞ?ës·ÎŸ?¯3‰âoàÞ?Á¬¼MÅýó?§'äVÐ?ë"Ð쎀ƒ?§'äVÐMIXED3FGL J0622.2+3747@eüãŠ	@%éW€•ÓÀ8¦'¿aª?À;…h9¥=<@4ڇöY
@èBæ.¢@Õ.=Ú¿Ó¤ÒrS.¦¿åcR§0ŸÊ¿îg
ɐ4õ¿ïþàf˜Ì{PSRPSR@€«5^ñýßPLExpCutoffLAT PSR J0622+3749?©_¤hE1å?°ŽÅL.?îj¹—)Â?°ŽÅL.?¥r
Z"ä›?ºlòûc
?î¨ß*PF?ºlòûc
?Ñ÷ß⠖?²¹T¡¢9—?篴þ?²¹T¡¢9—?ˆëÁ€?n;??´¸?ïœSðíéR?n;??´¸?¸†ø÷rô±?ěN<Ewü?ìï á:ܺ?ěN<Ewü?™Ã±"¨ú?³Ã2FpŸ?ï1âs°¯h?³Ã2FpŸ?Аâ»Ìtb?µe²@Tdù?緎¢ÅÏ?µe²@Tdù?M£«'??6EÉ"GL?ïø—<-i??6EÉ"GLPSR3FGL J0622.4-2606@m:†
¢À11 ‹ü"À9u™	PâÀ;Q­nb´*¿Ý3šfž±@ T^Q?ÿÁÀTCy¿ã-¥+ëb±¿àøÐ_Ã"ï¿äª!|&—¿"/YðóXäAGNbll@¡øøüPHPowerLawPMN J0622-2605?ïÿµ–¿
‹>úmh9?šT]Vm>úmh9?ïÇʵ×y	?ŽÖ@Ì mx?|¥«g?ŽÖ@Ì mx?ïê6lE?g
2TÓL\?eɓ¢(ÈB?g
2TÓL\?ïÿΪ¦û>ðoõ+ â>øª—!¶MN>ðoõ+ â?ïÿjFê¸?˜•4l:ý?·6q¢&?˜•4l:ý?îÎÝ?®
;?³Jˆ£ŠÛ§?£,ŽÈD?³Jˆ£ŠÛ§?ïåT
¬ç?sºæٜù?j«ãé?sºæٜù?ïþ3ì/'h?'@#À©Dß?,Á?|Å)4?'@#À©DßAGN3FGL J0622.9+3326@f~¿p@"P(ßó>À7_ÿ»6¢SÀ:¾t_Mm?ñmóþ¿ä@ $¥Z—ü@¿"|üÕÔ¿ßô,.©ƒ¿äʳ¿âÑ£˜˜_¿äŘQ´ÂYAGNBCU@ºXâeLogParabolaB2 0619+33?ïÿxV[‰ò?ÌÁPX'?õ2×NZ?ÌÁPX'?ヒ#¼H?"µ'¶D?€]?ò™p?"µ'¶D?ïÉȟQГ?}-yZò?{°7{Nx?}-yZò?ïÿû(æå8>¸PCjSþc>Ã\yhÏ>¸PCjSþc?ïÿ:³¸²A?"º«Óî?©ŠRÌ:Å?"º«Óî?îÍ )k3U?µ5îz°?£-ýf¹¸?µ5îz°?ï‡jgiš?Žª$"?Ž%f;Õ5?Žª$"?ïÿýs*;Š>·ˆ
F>´eÙºcˆ>·ˆ
FAGN3FGL J0623.3+3043@f͚€If{@ ý_çœ1À:,üۈQsÀ;«Ú
þ?ç#½É_ì@[ۓ9-H?þJ/ßÏ ¿ïÿö¡BÁ'?ïþ¨©Ú¼?Á¡í—÷'¿æ÷ãÃ÷€AGNbcu@°Ç–E¡ÊÁPowerLawGB6 J0623+3045?ïþåÒ˜?&5,Z
Ï,?&ñ¡S€'?&5,Z
Ï,?ïã7"¹,?¥EBғï?œƒ™Di?¥EBғï?ïÛ¬=V?kç·.¨|?r}*ŽÀ­?kç·.¨|?îó¡ï‡?Š˜š
ð®Z? Æ%ܼ½?Š˜š
ð®Z?ïøSußv?LÝ"úè-?N²+pMW?LÝ"úè-?ì-c4ªD?âtÛ/wM?¾"æ_"­Ý?âtÛ/wM?切ĭæÐ?"ƒNš
É?…ßÎÑ°?"ƒNš
É?íTøqZ$(?¯çƒê'H?µX<v
ÅÂ?¯çƒê'HAGN3FGL J0625.2+4440@e8OïI@,ÈFŸ ÂÀ9`+½,aÀ;'½ÝEÀÔ?–HDƒw@ºûø´\>@^È b¿älAÒæÊØ¿ãŠaçÚ"¿ÕÑéÝ­è¿Ý°6ÃOd[AGNbll@ üp£×
=PowerLawGB6 J0625+4440?ïþºõ×)"?›¯Ûæ3??$P¡`""6?›¯Ûæ3??ïËSGû—;?ŒÚ»oN¹Ä?zV\r2˜?ŒÚ»oN¹Ä?ïèѹÒ?eç–nWD?g.FÀ%ðæ?eç–nWD?ïñvŒªj?CLûÆú?]Ã_jÑ?CLûÆú?ïý"œAü?/Jy©•²?3_¼­?/Jy©•²?îú\%?±­‰"jÿ? Z>")1?±­‰"jÿ?ïÙ¦Wíþ?yŸŒ87Gù?s}¬àg™?yŸŒ87Gù?ïO*Nvõ?~Â9½
Vž?Œ¬5z ²œ?~Â9½
VžAGN3FGL J0626.0-5436@pu¨€QÉ÷À9ac€X€À9§Ú¥ÓdÀ;Áw=N?(?ÑÇÓÔ(
á@ã&?YÝ@]Ϡ׿ꬽo%–¿èñ2Á¸
¿åqh_åÿ¿ïþýR•gõAGNfsrq@s©îàóË>PowerLawPMN J0625-5438?ïúæ=¾ä?C"…ߦÝ?Dg‡3å÷æ?C"…ߦÝ?ï·1K–E@?=\Ü?'3­*<ãå?=\Ü?ï«ÀÙú]?wâlÉèN?…>Ï¢0Õ?wâlÉèN?ï{¾¶ÎL˜?qGûhéð?ˆ)Ÿfý?qGûhéð?ïødã{Ý?SHÖµ9ƒ?Oªl'?SHÖµ9ƒ?îˆÉMøm?³åóyß¿ï?¯‡slØG4?³åóyß¿ï?ïŒ+Å´2U?‡¼õÑ¤?ŒõŒ2Ø?‡¼õÑ¤?ë ['oP?©†©‡5Yw?Ã}Š'¶B¿?©†©‡5YwAGN3FGL J0626.6-4259@obY@x–À6hŸä6vÀ:!¾ê‹úuÀ;¥ðÍ]…?ôÁwAU
@¤f&O ?ûÖÁM½£¿æï"VZïT¿ÕËèÒ£ĿƝ_d‹è¿Óś¿}r¶AGNbcu@³dÝ/ PowerLaw1RXS J062635.9-425810?ïsz«Â»ý?•û"g?'ªŒÏê`?•û"g?ï3«ã+? 2©L(È?™Šƒž|úŸ? 2©L(È?í–ç‰ÖFã?¢¤Ø8VW?³Hò)¯è?¢¤Ø8VW?îÍWÍ$8?"©™I›2)?£*ƒ,âå}?"©™I›2)?ï:áߝMÈ?¡Nlþ
À?˜£Ä.Ý?¡Nlþ
À?ç7Üz6I`?ÏxEi§Ë?ѐG"mA?ÏxEi§Ë?ëøÛwEÂé?ª²¤"K¾Ì?À'"èô\?ª²¤"K¾Ì?ì8M»ìø?¨
Y¡ç-è?¾=' ˜?Á?¨
Y¡ç-èAGN3FGL J0627.0-3529@nnƒ¡	ÐcÀ3øÄ!HÀ8ÎFªß<;À;*½•!dÕ¿ÐÓT;ý˜X@=B´Z?ýåS ¹^¿ç'chP¿ÓS0¹±<#¿ÞE]i‰þ¾¿Ø @…~bAGNrdg@¢›¯\(õÃPowerLawPKS 0625-35?ïŽ6?z?½e@û·Šµ?Œxz²p!ž?½e@û·Šµ?ïÉ+}ºÉs?š¹ôÙ?{jA
M²Ç?š¹ôÙ?ïΆ­¦
h?xЛí;—-?x¼©4ˆp?xЛí;—-?ïûd'z]?2xÙ!CB‡?Cîn˜D?2xÙ!CB‡?ïêxÏþ
??|¤Œù	g?e‡0±0·?|¤Œù	g?î¾QOåÜ?µå¾Çaº?¤ëŽ6?µå¾Çaº?ï"¯NÙú?‹¥äÇ
?‹÷T%jI?‹¥äÇ
?ïÎÅ=y0?l£¢g¹™µ?xaX—<8?l£¢g¹™µAGN3FGL J0627.9-1517@lãø¶À(hß½jYÀ9óEî ÚkÀ;p©Ã³H—?ãÎöZS#@µú´¼Šµ@É£àDxÖ¿ãhD"œ™¿ï;Ât•dg¿Ù‡Èö?ÙÜç&•@AGNbcu@'Ïþ°t§PowerLawNVSS J062753-152003?ïÿ Ó/ù~?Ï	FNi=?Ë,x¤ÇJ?Ï	FNi=?ï­ø@†þ?'þzÉÆ?"ïñÏlŽ?'þzÉÆ?ïâÎòŸwÞ?`
@À'X?m1
[Âx?`
@À'X?ïüîüU.8?+'ƪcj?8ˆý®o¡?+'ƪcj?ïÿEÆf^â?k@ƒ^Š?G: ýøz?k@ƒ^Š?îDï"›?ºqɤÝ™?®›±~"J?ºqɤÝ™?ïzJ€ÏÈ?‹gur,t&?¶¯î´ló?‹gur,t&?ïð3òJà¤?_ã ·2Ä<?_˜Ïó'"?_ã ·2Ä<AGN3FGL J0629.0-6248@q{`(^ÄÀ:oc€X€À9ʉŒ\`À;ÏXK±?Íã¶ÑÁ\@ć®à~@Õ$@Q(ç¿ä}©kD,¿ãA'á2y¿âЅÛe…°¿ÔsºH!AGNbll@"¶a@OPowerLawPKS 0628-627?ïþ"ö0b7?'•B	‡ö8?&ÀŸª'áv?'•B	‡ö8?ïÅÊ,½?xºbú?}éŽB.>?xºbú?ïè?"û'?hTà!ÏÇ?gúÀ­ß¼?hTà!ÏÇ?ïçfYXê[?OiR€Ð*?h™¦:-²?OiR€Ð*?ïüŠÆ~:T?@ØpÂGŸ\?;©ÊÓ·‰Ê?@ØpÂGŸ\?îÚq=Yý¢?±;ÎǪ¢?¢Xì(¨WÝ?±;ÎǪ¢?ïË­eÜÜB?}rÞt¸	V?z)Mƒ[?}rÞt¸	V?îïsEÐwZ?H.[ÌÉ6?¡Ë¡@¼e?H.[ÌÉ6AGN3FGL J0629.4-1959@l"†_•'ÍÀ+Mûþé‹À7ý0T[¡çÀ;A0Kø&?íªJ
aµ@NkåuF@u'A8¿à
øe¤A
¿äuŠFHx¿àˆM-Ê¿ä"'J¿ä)AGNbll@‹¶Pÿ—$tPowerLawPKS 0627-199?ïÿ$I¥)_?%âÿþd?vÑêáò?%âÿþd?ï»h5ôX­?Ž0Óéhè6?%ò…QŽÂ?Ž0Óéhè6?ïÐÇÅÉDÏ?}w(¨X5?wœ)=?}w(¨X5?ïú,ûÐ_B?+ÆØMZ˜?GLôÀNX?+ÆØMZ˜?ïÿ8"ÍÛ?a·Cùè•?Øð¦¶_m?a·Cùè•?]àŸ¬?²¬Bñ²®j?¦Ç:†i@?²¬Bñ²®j?ï©/ú¢%¸?†‰Î;j?…´aÅeý?†‰Î;j?ïóÁ\‰ü?Jiw΄˜ï?X}H§÷'?Jiw΄˜ïAGN3FGL J0630.3+6906@b6`RP/@7b°ÿèÀ:ŒçìãÉÀ;úÌh"ÿ	¿ôßa.Ä
¶@
ÈÖ\˜‡@$ÇÛØX¿ã°»Ë·gпá´å]ÍÞ¿åR=‹7u¿êf:3Øt¡AGNbcu@'SÇE8ï5PowerLawGB6 J0629+6900?ï¤ò[ZLZ?žÐ²êH?†Ãi,܅f?žÐ²êH?ïÜs7IH?zGvóç—Î?qÆdgÛsë?zGvóç—Î?îà|ö†ë¨?'+¨<"¬?¡ø0"!©?'+¨<"¬?ïüՅ¥hQ?.JÇj€©?9SԗŠ3j?.JÇj€©?î²_>?¥¢iÀƬ?¤Þ*
âÅ?¥¢iÀƬ?îß̯ׯ»?µ6Ó¨ÖoÛ?¢5<ÒN?µ6Ó¨ÖoÛ?ìÞY¤X†Ì?¨.L¤¶g·?¹
2Ûñï ?¨.L¤¶g·?Ôàu)?Œný%jW?
½"áÙ?Œný%jWAGN3FGL J0630.9-2406@mí_‹ÎÀ-úðþÛ<ÒÀ7ßEó)WèÀ:°3cÛW?èÚ^t™I@—v2â*'?üó'_?€ž¿ËQú"Úgë¿Þ~OñQ^¿×¾!K²¹"¿ÓNÙ|ˆ'´AGNbll@¤<]²-VPowerLawTXS 0628-240?ïÚ|λB?ŸŒ[c@&?rÁ˜³)?ŸŒ[c@&?ï"ô=¡m›?—0¡‹ë ?‹ð¥c	6?—0¡‹ë ?îO9¨\ô?¡h‡Þ?5?«e}®µ?¡h‡Þ?5?€ëø·?nf_Rô`9?ŒŸº²þK?nf_Rô`9?ïŸÅëåŸ_?‹{×4ý^?ˆ…(Œ8?‹{×4ý^?í\kgpì@?º³Ìh×b†?µ¤Æž_|?º³Ìh×b†?Š\å´?žxämRhÙ?¤UG[
‹½?žxämRhÙ?íÞÅQû—³?›…ùU`?±	Õpÿ)h?›…ùU`AGN3FGL J0631.2+2019@hêßqêÿ@x€0¥À9fۙjZÀ;˜K»À5¿ä«—Y3´@st:9Œ¿@®èŸf7B¿åšqҚ¿éº€6œY¿á¿3]¿<°¿á¯hþ·_AGNbcu@"óIk¹Œ~PowerLawTXS 0628+203?ïþêݕ-4? ñ´`Ü
Q?!R%]z‡? ñ´`Ü
Q?ï¼å{ÅHI?"*ÀÌM?€Æ¡
N»?"*ÀÌM?ï¿cÒ¦D?d"GƒîÖ?€'=Ú̬Ñ?d"GƒîÖ?ïÿ¥¯Á=?Åähí?ëPkë!à?Åähí?ïþ*mÝö?4¼€á¡oC?-^é>¶óN?4¼€á¡oC?î£æÌI¼"?´ù¬h(¾?¥Á"=÷ì½?´ù¬h(¾?ï<#¥T@?›ÞñÂ+‡?œ8{†.
ø?›ÞñÂ+‡?ïõŠ'"kN?IâØÅ°ü?TêÛ\ÝӒ?IâØÅ°üAGN3FGL J0631.5+1036@i's`Iì³?Ýær¿~õBÀ7ö†
˚žÀ:ÙҢϣA@– ´Ö`õ@
ý6E'@?õ8{Çw¿ÕF
ë_¿Ý.×výk¿âžržzv`¿ìO^\#8âPSRPSR@'}ð‰ 'RPLExpCutoffPSR J0631+1036?Oç=ê°Þ;?TTû8‹Þ?ïø0"8?TTû8‹Þ?©ûúK¦–?ÃØDÉ¢d³?î`Fð2
G?ÃØDÉ¢d³?±A°…‹ž?¥´Û¯â³?í×Éï3]?¥´Û¯â³?™ˆØÄ6W(?zCš$×l?ï3¹:G?zCš$×l?R…Üèò?Nå²ÃJ³÷?ïö½{öñd?Nå²ÃJ³÷?"¾aqûi?¥¾«·'?ï­£sb?¥¾«·'?…/›B8?…ÃbjwP?ï«A".¯?…ÃbjwP?i	´ND?WB䕼 ?ïæ~缒B?WB䕼 PSR3FGL J0631.6+0644@i•¥¿­)™¿ôàÖ¿"ÕåÀ8"^ëGâÀ:–½öp4F?ù‡ÉûŒ'ì@ø'÷ŽÂ?÷­TF©1½¿—Õž'ŒŒÁ¿âà"~¿á7ɀ2W¿ìŒ˜_ö"OTHERspp@¤Oéº^5?LogParabola?"¯"j?ªýwÃ
º?ï['†ïŒ¯?ªýwÃ
º?¸©á}moî?À¼ޏ±¨?ìêÃÐXC?À¼ޏ±¨?ΌæåŸ#?±'Ä'Zyã?è\ÆF˜7;?±'Ä'Zyã?ÑæHzSip?£ö‡6*?çÛÂÖKH?£ö‡6*?P"#o
,x?Fî0P—mñ?ï÷µî†Ra?Fî0P—mñ?•–™ä^i?«5Â\?ø½?ïSK7r\?«5Â\?ø½?¡Ÿ…QD2?™©Ë[²§?îæªÝþg?™©Ë[²§?©þ >ÛOJ?Ž~z
[nS?î`üŒ›?Ž~z
[nSPSR3FGL J0633.7+0632@i£¿YFÿí»8 
•
À6ιƒCì¿À:Z֒Hl€@Ï)à#@Í@Vð9Žl@Ãë&Õù¿ÒSŽ:žj¿á0<<‹'¿æ9vTH¿í~Žè ÷PSRPSR@'UL˜_PLExpCutoffLAT PSR J0633+0632?V:æ'â£?YBS9€=?ïôâŒôçë?YBS9€=?£?•çjÈ?ÀSï~±'?îÌ¡¸T£?ÀSï~±'?ŠŽçu*à?©Îüo*?ï•Äbp­?©Îüo*?aZ@"?NoŒ±Ý•?ïí–F?NoŒ±Ý•?KçJ:·Að?AN4FÝ—?ïù-/|ß?AN4FÝ—?'eÕ D©?±zÄ?=5H?ïwdÑnz»?±zÄ?=5H?uð\Wo'?ióPc׀.?ïÕô:ò‰?ióPc׀.?9¢ª!Ö=ò?6Ql¥ú?ïü˪ãÃß?6Ql¥úPSR3FGL J0633.9+1746@hdA¿½ð'@'H$\À3L­áO:ÑÀ9=XJ@Äòýãñ@¶¥¹7™Ÿ?ôP'Ldë¿ÀŠ(æ¿ÚeR˜[߂¿ååðy+¿îA÷~§$òPSRPSR@Œÿ7`¿]yPLSuperExpCutoffPSR J0633+1746?-od@?èx ‹=?ïÿ·§û®?èx ‹=?¡÷þûYcZ?¾I¹òÕu?îà€!ú?¾I¹òÕu?…ϝ˜žö9?N³j›ÂM?ï¨Á‰fŠg?N³j›ÂM>Ÿmí"«>Ÿóœ­[ò?ïÿÿ÷4>Ÿóœ­[ò?+Äþ½z?%Ç^RÊ"˜?ïþC¯Øf?%Ç^RÊ"˜?‰yïáøù"?©l)0n+?ïš@NàÊ?©l)0n+?s¹ì¹YÜ?j½âqJUD?ï؍Ð14?j½âqJUD>}£h›"z…>‹)«o4{?ïÿÿÄñ·>‹)«o4{PSR3FGL J0634.7-2334@mû 1ίÀ+ýüߺ[À9£€)†À;ëˆy¶¥?欠tª û@?s­KÓ@JE Eš¿¿çm!W­TÑ¿åò¢ô@ã¿ëäTc ÿïÿL]?ýAGNfsrq@"ç4Á¨¬\PowerLawPMN J0634-2335?ïäÎjuƒ?lÑhÒFÀ?k1•VBqµ?lÑhÒFÀ?îÖs"¢8ú?¤y¿´è(?¢˜Æµ‰Z?¤y¿´è(?ï<-½IïZ?ˆHö+$wØ?˜zH[é~Â?ˆHö+$wØ?ìÎüœ•™Ò?'6×ÈøX¡?¹ˆí?'6×ÈøX¡?ï=î®Q•'?žA Ô6Ô?˜B*0¥ñ3?žA Ô6Ô?â€R#
;?ÑiT¥Ò?±?Úÿ[¹ÓåŠ?ÑiT¥Ò?±?í»¢Ó)?¦'øk'<Œ?·Ú'éf¶?¦'øk'<Œ?؍ƒ~Ø«±?°…B†5¯Q?ã¹>@"ª(?°…B†5¯QMIXED3FGL J0635.7-7517@qæG rѯÀ;)_JsÀ86
ÄÀ;•« éð?æÅ]‰ÀU@eºsY@®àI+m¿æ¶{v1ÏJ¿è]¦öh@u¿ë,͑Ôå[¿ïÿ.¶÷£eAGNfsrq@w…ÊÀƒoPowerLawPKS 0637-75?ïûSR.îL?C ý˜î+?B²¶Xû)?C ý˜î+?ï½r~o+?"öôÒÆ?€£`h²³Q?"öôÒÆ?ï€â"€>?%UŸcA?Ç^æÏ´1?%UŸcA?ïócñ'[?CPã-EE?YÙ7ÿt¹–?CPã-EE?ïùk'…ó?TÎq¿ïDu?JSa©£´ô?TÎq¿ïDu?ïY>¢Òþ??£šR¹ ͟?"Ø+¬p?£šR¹ ͟?ï<%ž†NŸ?•iÕ[¼"?˜{L*Â?•iÕ[¼"?ïÉH#ìU?rhFÇèG?~;[Ë­½é?rhFÇèGAGN3FGL J0638.6+7324@a¨ Àiçû@9¬OkxÀ9—}K…9À;ÝM×#gä¿Ñ{Ë6Žv?@.²§²Œ@笳¿æS<ã¹á¿éj;ÿE׿ä=š?\¿ïÿ©ü=RÇAGNfsrq@ju%F
¦PowerLawS5 0633+73?ïÿÑ á•>ùv^¦…>÷|"L.R>ùv^¦…?ïÝÎ&éù®?{‹1jQ÷?qìtU¼ô?{‹1jQ÷?ïß@ïÖ´?hVÿ˜<F?~0_'cyµ?hVÿ˜<F?ïûµV?*p±@-º?A+§¶ƒXf?*p±@-º?ïÿä¹þhü>ï	øø!>ëF ÍbÛ{>ï	øø!?ï.¸Kf?±-Xf&-D?š(ÿhi=?±-Xf&-D?ïÛn"ót?tmÃǚ?rHîñ6Ñà?tmÃǚ?ïÚ¸¤n+?hwQ:C>Œ?rð#·gÒL?hwQ:C>ŒAGN3FGL J0640.0-1252@kæHÿ¸²dÀ ŸóI"À9æ´5&RÀ;UHf¡?à9¶{#@
ÔÍLN?ø3@¿bÖå?ïò>Çøþ¿àV³üyì3?Ëò«{ã¿ÌŸÀÿRõµAGNbcu@ÆF§KƧðPowerLawTXS 0637-128?ïü"Êï?DwŽÚ¢p??W;؏a?DwŽÚ¢p?"ØûÀ?–Ãß9ø#‡?ˆ×Ó?–Ãß9ø#‡?ï°èɾ¶›?"9)qßZŠ?ƒǺãýc?"9)qßZŠ?ïñŽÐ½È"?F¦ ­/™I?\â^Ñfûe?F¦ ­/™I?ïñ€´#Y?`ʀnmJ?\þ—'åŽj?`ʀnmJ?í…Òô?Á'X¤É8?³Ño§`_D?Á'X¤É8?_o¯Ä?‰õ3[<µÀ?Œ( ¤s?‰õ3[<µÀ?ïæ—ޥߚ?_"H±œˆ?ih!Ac5¦?_"H±œˆAGN3FGL J0640.9+0752@i—]÷vÅ?ô}^?{kÀ9Ï!j´À:Í"4H?¸Vº£‰ÅW@
]lŽôz@rZ¿i6û¿äu§L
¿êÂ]B¡¿ê)^ž	¿ÑÒã|¼"OTHERspp@š¾"åÞPowerLaw?ïäEdă?tÆ	¾âÅ?kºëÃôn?tÆ	¾âÅ?{.Ó?˜8ï¶~#?‡›y"uÛR?˜8ï¶~#?í腩¼kE?¡%'b}™?°»Ò´BgY?¡%'b}™?ïæÞÞXw?U1è9?iÿ!çÙd?U1è9?íïú‡4?µ"Ԓg@ï?°‡çI­_?µ"Ԓg@ï?ìÿ'R;?¾®dÜ}?¸o¦¸i?¾®dÜ}?éCVbH…¼?·GŸ'­?Êò¦vÝé?·GŸ'­?îGÕúrøE?¡•Idä5h?«' T"ø´?¡•Idä5hAGN3FGL J0641.8-0319@jÙ¦ %9uÀ
gßbP­À9‡86¨2ºÀ;¯#nš?çÞKpåW@¬¡ÚZÔã@¢Êi²K¿æZ×ä⣿ã=*É(å¿ãÀãîZÙ¿ïÿôG÷ ÅAGNbcu@Šv"Fs'PowerLawTXS 0639-032?ï÷ª@°Ê8?qnÂø?P«~¿gÐD?qnÂø?ï€3³Y?¡'"ìC?ÿóJ!ý¥?¡'"ìC?íT'M恙?£ËÝö+X?µ^ő§Ú:?£ËÝö+X?﬚¢Ùo?cB\©ø¯"?"ÙWI½ä'?cB\©ø¯"?ïÛEiö?Š
È3tœk?rv]XŽu?Š
È3tœk?ìÎGŒ9<j?ÁQi¹ÿ?¹ÃœìB0?ÁQi¹ÿ?ì\#!Ρ?¨Øá?5û?½ç>ñŠû?¨Øá?5û?îk?û(æå?•e"<4$$?©LPF©?•e"<4$$AGN3FGL J0643.2+0859@i®ÀrKw@:ßkàÏÀ8dbzÀ:ÎÜq…~?ùûdg@Ú3më–@ÜN®¹¼O¿Þÿi;Ö¿ä»`ã¼õ·¿è|s±±¿ïÿ…"
ì'AGNfsrq@‰—óÿ¬*LogParabolaPMN J0643+0857?ïƒg.?'ï§ÐæxJ?=&FÓ³x?'ï§ÐæxJ?îj–Á´&?·+ã–dq?©^֓֟?·+ã–dq?çà@‡"™,?±ƒ*Ÿd?Ð?~ðöͧ?±ƒ*Ÿd?íoùçÚf¶?'Îûapïh?´€0Á,ÊR?'Îûapïh?ì
Á£à?½~05ìÐ?¿—Aòá?½~05ìÐ?ç«'-–f3?˘2JnÒà?Щ±¤Ó3™?˘2JnÒà?æ+ï"T/z?¶DÅÖDh?Ó¨ ÷W¡
?¶DÅÖDh?èp'a´Œ?´õýÊP?Î=»Þy-Ð?´õýÊPAGN3FGL J0643.4-5358@pu3?ÈlìÀ6ÆfÙ×À:
Oa´À;Ç1Xg "¿òó—Œy§@Ùê†7"@Œy¦Žu¿êN=ÄAôþ¿×%ƒˆÇJ"¿ç½z_þ©z¿èñ04;AGNbcu@xÊ#9ÀìPowerLawPMN J0643-5358?ïöä%·}8?T~ƒÞÝH®?R7´ÒþË?T~ƒÞÝH®?ïÌþ)]"?‰8{íBUh?yÿóF?‰8{íBUh?ï~J4ùÔ9?ŠÙ%ùùPš?6¹[žÞ?ŠÙ%ùùPš?ïÿ"Z ¾?3þÄÞ?é[–N°&?3þÄÞ?ï즳wU?o3ÐOUÙ?cYL'IØ?o3ÐOUÙ?ï,«ã¯Mœ?®Dµ³øã?šjƒ…èv?®Dµ³øã?îÔaM;·?—KQ"ynM?¢¿Éìä?—KQ"ynM?ïö¤6dÊ?IÌï¾?å?R¶Æ¨9?IÌï¾?åAGN3FGL J0644.3-6713@qX—ÿ›V2À9‰4ŸCý†À7ØýCŠÀ;åÉä?ìD™ùw@Ou¬ªm|@ÂÿýfH¿àý'²Ìq¿áæ
n £¿à½ëtœxá¿åS
æ&ÔÅAGNbcu@ÎOv_Ø®PowerLawPKS 0644-671?ïÿ?^˜D?!jÀH¯«Â?X¤um{?!jÀH¯«Â?ïÁ둫[?'TwPáâ?v
9:{?'TwPáâ?ïÎà÷Pò?{,îW¯fý?x"R¶Ð?{,îW¯fý?ïþ~g±a"?BÓK£ï?(ßsz½?BÓK£ï?ïýÞ¿,j?8£Ývk?1
\êJ²?8£Ývk?ï•$¦
×?³Ø¬TÙÇ?í[r}	?³Ø¬TÙÇ?ï³ÌB¹8?‡¤ÕgX²?ƒïSÁ½_?‡¤ÕgX²?ïý‹Òԛ?- ¢C"7š?3§Á¦íÀv?- ¢C"7šAGN3FGL J0644.6-2853@mÏ:ÿ°NèÀ,.z WŽ\À:_Ï2ÚÌÀ;Ä}‹F¿×{ٌ›%Ø@d‹šÓU}@㦿qð]¿ït¾§VVà?å	k©qRþ¿Üù»ŠA¸¿ëP"T'±AGNbcu@¢ø`IQƒPowerLaw1RXS J064444.2-285120?ïÆiìWׂ?~Psµ*V?|Ë	Å¥âå?~Psµ*V?ïÀ¿êªò÷?K°{µz? 
˜¨ŒŠ?K°{µz?íòOÇØ5%?¡Ò;x[nV?°mÀboÝ?¡Ò;x[nV?ïñRz÷#?K¥(A:+?][	¬J)?K¥(A:+?ïÂZo¯‡º?€}¯lq–?~ÒÈþS%?€}¯lq–?îdNjŒ®?·pB®Ü?©»_N?·pB®Ü?ì|òðã?ªžN,"Ÿ?¼Xhxå?ªžN,"Ÿ?ïwÌ&?†=Ð¥?'oÈ3Ð?†=Ð¥AGN3FGL J0645.9-3914@o@ßXÀ‹À1À¶àÒ=OÀ:ª>,‹À;Á¦V]ÛÀõ‹¾åƒ}@Ê'D½t@'ù gÔ{¿êI»üke¿é
šO±™¿å«¤¶£¸¿ïÿ1¾¾íAGNfsrq@sóO"}ŠPowerLawPKS 0644-390?ïúÅËü˜A?D-™*~?DèÐa»Ïò?D-™*~?ï˓h6[?ŠÒçw?z6pT#â>?ŠÒçw?ïfZ"}J%?€Õ'ÆíA?"4¯w5óU?€Õ'ÆíA?ïÿùÝŸE>ųÒvdˆN>Ȍ7
·D'>ųÒvdˆN?ïùš‡ø~Ï?IބÄúêû?I•àq!ˆ?IބÄúêû?îäQ:| ?²Wè
26s?¡ºìV~1¡?²Wè
26s?ï,ô½«;?'1±ëÚ`?šahV©ÐŒ?'1±ëÚ`?ïþöé^†|?#µ+qyÐ? 'iHâøÎ?#µ+qyÐAGN3FGL J0646.4-5452@p†Z\FRÀ6˜À§¨À:±Œ7±G5À<w&0ì1?öaÖâOj÷@!VØÿ¶¿È]¢Pþ?ï¯ù͋äz¿ÚՕŽ7ï¿èÛ~re'ï¿ïþÞdFHAGNbcu@™ªßØ­«ŸLogParabolaPMN J0646-5451?Ãs§×õÊÈ?ÎzÔ lö½?ë#
N?ÎzÔ lö½?ßÚm>œÈÎ?ÒT¼j~ùÛ?àÉ`±›™?ÒT¼j~ùÛ?ØÓ1ŸÂ?·'zg£rù?ã–gp°õ?·'zg£rù?ØÕuF—ؾ?¿Újð
ï'?ã•E\´¡?¿Újð
ï'?Åm²5ë™?Ôó‹•tƒ?ꤓr¹?Ôó‹•tƒ?ĵ£K°=Ü?Éч'?êҗ-ð‰?Éч'?ÈÏuêה?´Wp.÷?éÌ?b…J?´Wp.÷?«Æj\:§?¬½…›°¬?îC™Z.Ÿ¦?¬½…›°¬PSR3FGL J0647.0-5134@pOø!ïÀ5"Ð_ÿDÀ:C*È*§À;ڈ§ÙÎ=?Å$ÿÇSš@
âÖ¤fý@ƒâ?Ð¥t¿çÈÓ*^¿æb5a¶©J¿Ø–8¥³%¿ÑyFðKÏYAGNbcu@šÒ•$ÝPowerLaw1ES 0646-515?ïÿ&½?LW?ogˆhì?(Zœø^T?ogˆhì?ïא;2A?ŠM^£Ê?~47Ä*O~?ŠM^£Ê?ïæ¸l~¿Š?cH&ù«µu?iG"V¥Ng?cH&ù«µu?ïî%ƒXuÉ?G­Rî?aÚ|µH¦×?G­Rî?ïýÓX¾CX?3=ßg \?1e9®<ê¥?3=ßg \?îtbÄà-?³½%µü³?¨¹Ó¯kÈ8?³½%µü³?ïͱ9Ú}v?y;Áà?A?y'c,ÞM?y;Áà?A?ï_%"@cj?†83,?"OtƒöÊ?†83,AGN3FGL J0647.1-4415@o²Í ¯¢ðÀ3I`ÆuÀ:œç+ó¤À;ÙLhÏÍ?¼ýaÄYûc@]†ÎÇ8@Ás\f³¿ìôyI˃ª¿åÐhYíî?Æ ?ïìÒRzÌ$AGNbcu@"¾õöý!ÿPowerLawSUMSS J064648-441929?ïÙjўÝj?pº
ß:r?sJ—E.òØ?pº
ß:r?ï¶ðà…ïÌ?Œ£yUý?'CÇáC¼ï?Œ£yUý?îÑjžââ?ŸüL`8¡?¯BéS~à?ŸüL`8¡?ï¾Szç?p€êFÀcÊ?€k:½',?p€êFÀcÊ?ïoY+ë@U?—"©t?'چ'P?—"©t?í£x6ŒGæ?»BP‡éû?²ä>Lç›L?»BP‡éû?í[¾'v??©Ð»Ý¥Ý×?µ"Ľ)"?©Ð»Ý¥Ý×?î›&ýÎU?¥›ú1ï?¦M&ŠJ ?¥›ú1ïAGN3FGL J0647.6-6058@píοìºÀ7ñàè@À9KTÛúg:À;­ÈŽyªç¿'t8w÷@ŸŠùB̃@±¡ y1ſޟÜaÈÐq¿åd'ït¿ä3Æ£_c¿ç,=¾&–ÃAGNbcu@‹
"FsØPowerLawPMN J0647-6058?ïÿ{ËS?¿³Gó=?ŸÀ€3,Â?¿³Gó=?ïÁ|=ÿü?'ÑD˜Å»	?AòÔ¡j?'ÑD˜Å»	?ïÜî<«yb?qÊ4b!y?qˆáœ"Þá?qÊ4b!y?ïñ\˜ø›?CE'"ö-5?]G‰"?CE'"ö-5?ïþ®Ü÷?)‡ñ96m?%.Î%³Ø?)‡ñ96m?ï™eʽ²?«ù—+çJ¹?ÌÓDð{Ò?«ù—+çJ¹?ïŒi©p¸?‹¢×Ûɕ?Œåºœƒ	Þ?‹¢×Ûɕ?ïppÓB?~0&a´=?'ñåšñÈ?~0&a´=AGN3FGL J0648.1+1606@hÅZÀ?ö@A.Àë­À:…Ç7bÀ;±'[¶¿ížðÆ|&@SöâŸòÏ?üdÞßHûG¿ë\Šfd§¹¿æ̶Êàl¿ØHZ¾"Ì¿ÝOŽéðÓAGNbcu@À"ùÛ"ÐåPowerLaw1RXS J064814.1+160708?ïÿ)ë®0Í?={'Ò¬Vl?'œõ©?={'Ò¬Vl?ïÆq{9Ԅ?ˆî}
g™	?|ÇB^ö5Ì?ˆî}
g™	?ïân$©`??p^mPìÓ½?m'Û.ÄI€?p^mPìÓ½?ïÿ1²ïDá?cʙ?É¥3oÎE?cʙ?ïÿ1ÿ<È?Þ?@ çá?YÀc+T?Þ?@ çá?³áÌí?µÔ¬þÆÝ?¦e¤Æ.´/?µÔ¬þÆÝ?ïލŽa|?tWþ?EÆ?p¹9®yñ?tWþ?EÆ?ïñíÏb¤?[…UÅOo?\$`Û­¨T?[…UÅOoAGN3FGL J0648.1-3045@nÈ˒:À,BIÿ''ìÀ8áfãcèÀ;rÍ 1cO¿¼Ü+Ë­4@GÜ7£Û@te€¿æ#­5F¢–¿èZçï+á¿ãHþ®òf¿è»zóoAGNfsrq@7H@áqŸPowerLawPKS 0646-306?ïÿÍú¤'>ò¦œŽÈÞH>ù•Sí
>ò¦œŽÈÞH?ïÂ1©Mõ4?"]'v™8?~ç+:ê-?"]'v™8?ïé€~·ãS?l;YN¦-]?f;¾ù?l;YN¦-]?ïÿåZ"¨=>Ùß©%Iã•>꥚YZä>Ùß©%Iã•?ïÿ®ý0?á&1?yoõ¹‹?á&1?îÈpü—k?³D3óûÏj?£8ñîWR?³D3óûÏj?ïáð=Íä?s©Ew?n¡jëQ?s©Ew?ïÿ¬
_l?Á‡9(/?ýWŠEl?Á‡9(/AGN3FGL J0648.8+1516@hߚŸ¾vÉ@VÚ`SaÀ8ÄN¨¿¨À;ÚaàŨ¿èÞn3ÔÂ@­@͵€?ýKF(_?ÍF:™Pjô¿Ôl.[ ü¿¿×``¹Û¿Ù-Á¼î‹AGNbll@­\6¡aä÷PowerLawRX J0648.7+1516?ïîRCÕÔ?g-ã<v»?aï­¨ì\-?g-ã<v»?ïÂÑòâœS?Š(s8GI_?~—v¤'•?Š(s8GI_?ï[WÁªQD?ŽÖqÆ•Û?"•ÓLÝm?ŽÖqÆ•Û?ïü6†=¶?1—úeéø?>KÌÏÁ?1—úeéø?ïÃÞÙ©í?/å"Tg#?~"aeŠ?/å"Tg#?î|iùKŽ|?¶ …·¦"?¨9`o'›4?¶ …·¦"?ï'/n?–1^¯©I'?›Ùõ?–1^¯©I'?ïÎøÑbˆ¶?rÆæt	Ýd?xƒ—0?rÆæt	ÝdAGN3FGL J0648.8-1740@lŒ`Ëò²À!9ÿÖ•À9aéÐé'ÿÀ;%HŽå?Éoà<+ø@¾ß"	v@(Mß[ð—¿è`.'ô¿ãÉç'/y¿éѼø»¿åº4!xSAGNfsrq@ŠpãŠ	PowerLawTXS 0646-176?ïÿ¥)xR?.iìXd?)?«ZÃÄ
?.iìXd?)?ï¬A øø>?–è3V?"ï—Å1Œ?–è3V?ï¸5—ïÿ?{\aÂ?ÿr"" P?{\aÂ?ïüüÖ]wÞ?³ÐÍxN9?8KÈ3Ÿl?³ÐÍxN9?ïü:9He?NÂUxß?>.3í›r ?NÂUxß?îPÑo&‡?´>ëèºÌÂ?ªòé+D?´>ëèºÌÂ?ï8¤5Ì7?"uNê&'~?˜ëyK †V?"uNê&'~?ïìép­£?U~D+c"?cbÏëY?U~D+c"AGN3FGL J0649.6-3138@n06¿DNÀ,d:a$ÞÀ9¬þ›{ñéÀ;`œ
è ?ͯzVˆLë@¸±¤þ&·?û¨² yL¿ìýkÆLªþ?Þý*ÍŽØ¿Ãsýyy#é¿Û­fѬk¿AGNbcu@¶Ct¼j~úPowerLaw1RXS J064933.8-313914?ïý´þœJ?0×â4x¤?2X
Bá§?0×â4x¤?ﺚßPW?'?g–^ž?YH;È
?'?g–^ž?ïØnèV?rCIsp?sȸCêlÆ?rCIsp?ïæ…KŸ¤?O‰¿ži™æ?izµ¼sÓ?O‰¿ži™æ?ïôô±mJÜ?R'é>W?Vnõ?R'é>W?îG4…ÔÑå?´»*ÞX™?«Œ· ,²?´»*ÞX™?ïÂmâò?^ÉÑP-U?~É–F?^ÉÑP-U?ï‹	LÉ¡
?zß?+•?=¬Í—¼¹?zß?+•AGN3FGL J0650.4-1636@lv²gÇÀÓþ_ìÏ¢À9.Wø™÷À;Æ폺ô?ðûc"xB\@håòŽ@uâÿi,>¿ÚéÒU'›¸¿æ[xt
¿é€îIõ˜¿ç¯£2ìÞ²AGNbcu@¬
Oß;dPowerLawPKS 0648-16?îlœCn?³HÅ̐ò?©?¦;Ç	?³HÅ̐ò?í–;ë×?µ9ó@ÔÜf?·óN'¡I?µ9ó@ÔÜf?îˆOQÌÑT?šâÆh—‰˜?§{
àŸ5½?šâÆh—‰˜?ë'·ÉÒ?"H j´¢á?ÁôÅàۈ¹?"H j´¢á?çŒy©î?Îk¹;ÔË?ÑÐç­Ò%?Îk¹;ÔË?Õï@Œ"€?΁•<pQ?å@_¹½À?΁•<pQ?ç:Âé@˜C?·Òù6I¤?ъz-~Ïz?·Òù6I¤?ØG\GK•?³
ó´¼6‡?ãÜQÜZx5?³
ó´¼6‡MIXED3FGL J0650.5+2055@hA}`éNä@"c.Àë­À9¶'Ã]À;Th®?C¿°[5ÑÎ2`@«–ÌŠ²¡?ø@W¿ê»b‹TKK¿ØêpY·ßÞ?›FAi#¿Âôû#ÞAGNbcu@ÂBMÒñªPowerLaw1RXS J065033.9+205603?ïþ*§ÀÆ&?(E×ÛDUŸ?-Uò¨­?(E×ÛDUŸ?ïÂl'ùÞÃ?Ž{»bA=¸?~ɾ°Æ¾?Ž{»bA=¸?ïÛÈ~Ŕ?rN•×>o?rÀµCA"?rN•×>o?ïþ¥'@ý?µ½±¯{²?.媵µ%?µ½±¯{²?ïö\Éb<¿?R–y'²?SFl½ãZ?R–y'²?îÄ*‹ç Ø?²Ísa‡À?£½WDýŽu?²Ísa‡À?ïÈëuü¨Õ?€¶ÿÝý–?{ŠDúÌ]"?€¶ÿÝý–?ï÷Tއ<þ?H îæw€?QVBÍÊ°?H îæw€AGN3FGL J0650.7+2503@gȱ ‹ü"@&ðál—À8F-ù7ŽãÀ:мž_ç¿ÞÂrYzH@ 9#¸?ûˆ~žìiË¿Ób"ý[>¿ÜυÜé-¿Ð¦=Y°S"¿Ôà©3¦²AGNbll@¬T¹Û"ÐåPowerLaw1ES 0647+250?ïý!³{dr?.WõaT¯;?6òd¿äjã?.WõaT¯;?ïÌӗ0! ?ˆ,‰Ö'?y–4{-?ˆ,‰Ö'?ïÄÿý~î?€½#<À,°?}€i¢á
?€½#<À,°?ïþ™N¬F¬?PC1- Ë?&kòE?c?PC1- Ë?ïøW|銞?Qüƒ>ÓkH?N¢&´ó??Qüƒ>ÓkH?ï3A Ú?­Zš}µ±?ù—á&®½?­Zš}µ±?ïËÈfœÓF?" õ"ߦ?z̖Éi?" õ"ߦ?ïõïÌ3ÓJ?LûwUÕHa?T ghm)?LûwUÕHaAGN3FGL J0651.3+4014@eýÓX"@1­ _À:«õ¼°À;ËÌ%ÝàÀlæ.D@ø{
bZ@õþ€y0¿ÕOÌÔâùh¿éùIЃ'¿Åš—ùäæ¿Ünf¶©†AGNbcu@ 3A‰7LPowerLawRX J0651.0+4013?ïÿ¨@È¿n?0r#×?ïÅûƒ:?0r#×?ïٗÝ%ƒ?'¼U쨭±?s4}Š¡?'¼U쨭±?ïë–Ögx?ZzÚÈ«-?diå;0v?ZzÚÈ«-?ïÿÿÂB…6>†¬ÃA"•>~ë´ÂVöp>†¬ÃA"•?ïÿÀF…V>ý,þT³æ>ÿÜÕ5ø%»>ý,þT³æ?ïXéöÎÊ?£\²-Æ)?"âÁ=½ôÄ?£\²-Æ)?ïïzQ)é3?a×Ðü§Có?`…®Ú6Uq?a×Ðü§Có?ïÿü"Œ>>ÃnÛÔj2>¾ìz§åI>ÃnÛÔj2AGN3FGL J0652.0-4808@pQ?´‰À3ÀÆ3¡îÀ:iñxôÀ;×PÁ¹sT?êº°‰íw@
üxŒØ@Z"`Ÿ§ü¿ëœ†ÀŠ/¿æf1ýþóæ¿ÝBÛB—f?œ^yæ~'EAGNbcu@©H°|"µÝPowerLaw1RXS J065201.0-480858?ïù@ÒÇÒV?Mг"±ž?Jü´ê1ï?Mг"±ž?ï©U¹´±?'¼±3¯¨ü?…¿*Š³›Ð?'¼±3¯¨ü?ï›ø$z™à?…}BþŒ·?‰öӛ?…}BþŒ·?ïɬÝKӜ?gFšà•ÓN?{)'_•'%?gFšà•ÓN?ïò˜iK{²?]B—UüÉ°?ZÏ-»;'?]B—UüÉ°?ët¸—>S?Åu­êg?ÁÊ-£³?Åu­êg?îØ8ȕÒÝ?›Ø¶ë$Å?¢|sw~¹/?›Ø¶ë$Å?îM2W™?¢ç6Z?«,ڔ
¹l?¢ç6ZAGN3FGL J0653.6+2817@gqXf€@)Ú'ÿ"ŠoÀ9£/…(ÉÀ;¶ÄnYyï¿þK_§…jŽ@èžd"@ÿâ'…¤¿è\Žab'¿ã55¬E¿ÐuÛӔ«ã¿éå¡9ËþœAGNbcu@"&i*0U2PowerLawGB6 J0653+2816?ïƒ['eS?¾=ÉlΒþ?)púM?¾=ÉlΒþ?ïÑé¬#'?‡j"í?w*Ì"?‡j"í?ïŸuø:õÛ?ˆ…¸R3?ˆ"û']?ˆ…¸R3?ïÿív¦¼>å3›º‰h©>âŠ	7,x¶>å3›º‰h©?ïȧJv	¶?}cÚ)õß?{¬ZΚÊ?}cÚ)õß?îôÁ¹Úgü?³öyhV? ³äc5g=?³öyhV?íèk$Õç?£Œf àð!?°¿4¨#+F?£Œf àð!?ïþÆeeƕ?'uk*ˆ?#™«÷†'N?'uk*ˆAGN3FGL J0654.4+4514@efŠá'6@3cS`Ð$pÀ8ºp©¶À;Vä'Ë÷»?ì²*3Uö@Vn=Í@L_ß¹Ž'¿á#±¿å0ŸZ"á¿ã[ù¥óÅ	¿æ¶ÿNAGNFSRQ@"DZA_EáPowerLawB3 0650+453?ïÿ'…£î\?õC=î8?ž›éú%?õC=î8?ïÙK–p3?'™æ'?n?swÚ4úh?'™æ'?n?ïäñì†?bß$Mr:¹?kb€U
U?bß$Mr:¹?ïÿÇêv:>ëX­ /š>ü
ѯ³i>ëX­ /š?ïÿfƙ¾?e9ցð?'47FˆG?e9ցð?ïóºw_³?°Êȵ—Ð6?aˆ²Ë× ?°Êȵ—Ð6?ïÀ­‰‡õû?'/vÿ%Ž?©;Js^¤?'/vÿ%Ž?ïÿ¼÷uJ?¡ÜKÞ?ÂñBžö?¡ÜKÞAGN3FGL J0654.4+5042@d¶êá‹@5w ÈÍdÀ8Þˆò'À;y\*£A¹?öŒ¬KMl@<³µ¥?ü¢õ°pÌ¿Õj=p£×
¿àËp¶÷M¿âmX•dοæþŽÆÚ
AGNfsrq@Š÷˜âe,LogParabolaGB6 J0654+5042?ïþ{ZCÁ?(EN8ƒ?(Jc¿ìEö?(EN8ƒ?ïÆ@X¿	?‡Ç?×÷ÇN?|ßûä·s?‡Ç?×÷ÇN?ïF¦V…6¥?"š‹‡EÅ?—+52ÈÇ]?"š‹‡EÅ?ï¿a²Ö	??_d'¦¯÷ë?€'"W4>&?_d'¦¯÷ë?ïú/×:?Gq •Ý—?G—A‹Q"_?Gq •Ý—?î³9´<ï?µ®%-;A?¤Î¬cc?µ®%-;A?îئ-aô"?›œ°û5?¢u,trÜ?›œ°û5?ï\ü€w<U?'Æ+¬Z?"`oèog?'Æ+¬ZAGN3FGL J0654.5+0926@i›``þG™@é‹@•À9ÁÃèø|~À;]²_c<æ?ÔS~"|ñ@þP
.'@S©"Ð\¿à"Câ¶v¨¿ê-ûL&¿êÝQõk&•¿ïÿcÚ½GÁAGNbcu@'±XbMÓPowerLawRX J0654.3+0925?îŸZ™‡-º?ÃêµÏôä2?¦
Vg$c?ÃêµÏôä2?ïcÑIðJ?¤{xLfØ?"ÅßXü­?¤{xLfØ?ü
¹(?'¿¦›ºÐ?¦ä Aè"?'¿¦›ºÐ?î˪ßü?€Eú©q?£E^¬NK>?€Eú©q?ÿÛܤ?"NÄõ» ?Š[¿þº?"NÄõ» ?芒˜H‹µ?ÉéqjÐ?ÍÕµžÝÑ,?ÉéqjÐ?í
€nû5k?¤Ÿb'ߺ]?·«üŠL%?¤Ÿb'ߺ]?ã"Õ»;ˆu?´ÝšÆ?ØØT‰ˆï?´ÝšÆAGN3FGL J0656.2-0323@kÊ¿ÞñßÆ£'À8NAûMØÀ:Óïµ/!V?ûÇwB¬¢á@ö{ÐÛÐ@lj
µ¼¿Þ…!vŒ6¿æÔ<k§T)¿åQÇ™8e¿í²ðF"QAGNfsrq@‡¬8ºÇËLogParabolaTXS 0653-033?ï­- !H$? ã
1V?"´—éï‡? ã
1V?íyþî ô0?À"¯$£Öè?´0B8ý?À"¯$£Öè?ëRFaä!?«Ãw<??·Šæxo}?«Ãw<??ìéBvO?""¬ßlm¯?¸µìK…I?""¬ßlm¯?ïÝy\&5?éi‡ûXô?"PÖ3Q?éi‡ûXô?äúNxDF?Ϻ"WhÐ,?Ö
ácwu?Ϻ"WhÐ,?ëHÚUæ*[?¯kÕ½Á?Âܖ¨gV•?¯kÕ½Á?çåѲ¡?´ß¸ÚÛ?Ð4]ò›à¾?´ß¸ÚÛAGN3FGL J0656.4+4232@eÀâ€'،@2жâ—À9¤ÛÍÐfÀ;Ÿ<zڑ±¿¨›æûÍr@=¹±¼ûô@œ3`ª¶¿áÔÒKfÜ¿èäbÉ+‹¿Éß´à5Ï	¿äúµÝ`ÝAGNbll@D¿åÉPowerLaw4C +42.22?î˜þ½põr?ÉfºÅÊ`G?¦p&\óç?ÉfºÅÊ`G?ïËÔc]â"?ˆáð0»Dö?zÎ6Aû	?ˆáð0»Dö?ïÞdºÈF?y(qœN!›?pÍ¢±Ú{â?y(qœN!›?ïç}9‰?Qsíf¹9?h'ÆE€‡	?Qsíf¹9?ïû¨ºýJ?TÈ{d¾[?C‰\rj*?TÈ{d¾[?î¸?Ó?´þºÞ\U?£ß¤|òÊ?´þºÞ\U?ïZ_á¬?†×)Hò]?~¹RºÁ–;?†×)Hò]?ï>_ýý­|?Œ#ŸPï"þ?˜4G)ˆ…?Œ#ŸPï"þAGN3FGL J0658.3-5832@pË¿ƒ8.À6…rÀ:cþtŖÀ;×~ßÙïË¿ûa
Œ±@`Ï«¤^@7(`Ff¿ëM:£óm¿ÎK6Ù ¿ë÷"Èú&Å¿Ô;aSñ³{AGNbcu@šì"h	ÕPowerLawPMN J0658-5840?ïï·¼?p¹-ç?`øê0æŸØ?p¹-ç?ïÓÒûe¦?"WöIe,?v'1úÍ1?"WöIe,?ïHŒýY?Š'³6Ǿû?–î`TÛLã?Š'³6Ǿû?ïÿނ+é¾>èbÆRJ߄>ð¾ñ¶jÓC>èbÆRJ߄?ï"3['?¡ °ƒ"Ü9?›¹œM»æ?¡ °ƒ"Ü9?ï*¯£h?±|ybTyx?žª³´q?±|ybTyx?íf0
+I|?£Ü¹À/Ï^?´Î¬íæ ?£Ü¹À/Ï^?ïù`T18:?M݃å©á(?J~¯!Õ+Ó?M݃å©á(AGN3FGL J0658.6+0636@iûg_ö	Ý@_ú D®†À9¤Ï©öÞïÀ;Y#)гâ¿ÝËY'¡@ãA¯¢Åg@ØeêV ¿èí¯½¿¶¿âî`<Î	¿çq¥õ¢"¿Ý'ô)¢AGNbcu@ŒÄÓ@N¤©PowerLawNVSS J065844+063711?ïõKî.á?c(˒ó\¸?Uh#ä6yý?c(˒ó\¸?ﵦ­Õ«?HP'•?'–T­»Á`?HP'•?ïcèBu?†l=ÉlΓ?"'îÒ%Ë?†l=ÉlΓ?ïöôE.)Ö?=çݚ«¯Â?Ru«ëc5?=çݚ«¯Â?ï´4úL{?†!c!ï[F?'òÁ{ÿ`Ž?†!c!ï[F?î3§¾à?µ'Œ?¬Å!Æû?µ'Œ?í¤ÄÕ~ïl?¤JÊ†á?²ÙÙSš'#?¤JÊ†á?ï?k#JÄ?1çåŸ/?˜›'€p?1çåŸ/AGN3FGL J0659.5+1414@i"‰€²B@ oNó[À8I?>Ú0cÀ;_ÆÞ?ÿä+mìí@ëäj"^@
ùٕˆ¿äÛUiú¿ìZi}že¿ì­Tcuv¿ï5IçÙ"PSRPSR@mö½f'|PLExpCutoffPSR J0659+1414?—}ÃC'i?£ÊJÜy?ïDè4Ý,?£ÊJÜy?ª¥²îli?ÃV
­°A?îU®µœZ?ÃV
­°A?ášq}=?³tßš|Ã?ÝãÀˆ?³tßš|Ã?ŽŸØÝX3"?}VÏ|Jðf?œacâ?}VÏ|Jðf?¿0Mî¨ó1?¼ƒ;¼Í-ù?ìöB*áš?¼ƒ;¼Í-ù?Š=Ò`™û?¡°svE?ï—çÑúx?¡°svE?â ‡*Æ?¶-óz?ôþ?Ûõ¿Üñªt?¶-óz?ôþ?V6M›öŠp?RI«›Rïû?ïôäÙ]ÿ»?RI«›RïûMIXED3FGL J0700.0+1709@hÏ_¿ƒ8.@#. ÿê[~À9O7¢KðÀ;}x–ê'°?îÕÇOèÔ@8Ej˜O@Ÿ 䨿刻®tü¿ê"m/¥¬¿å
îޚž¿ïÿœ¹šÒAGNbcu@€Æs×ÜPowerLawTXS 0657+172?ï³ü—?'Ô'žÂ?ƒú"s >?'Ô'žÂ?ê^ÊKú:ª?¿òÛ:‰úÑ?ƄÖÐW?¿òÛ:‰úÑ?î<£aá?œ°bLÀë?¬>eÇS<ó?œ°bLÀë?é@À?~MÁ?šél£?ÊüÿÈû?šél£?ï$<•‡'.?¡Ó÷ô¤ÊS?›xmR}v.?¡Ó÷ô¤ÊS?Öd9¼\?Ð*2ƒŠä?äðÍúc!Ò?Ð*2ƒŠä?éèƒj5Ü?µ<ÊøS'·?ɼ]òW(Ž?µ<ÊøS'·?ÑSøÜ[qQ?¨÷"Fû?çV'ÒGW?¨÷"FûMIXED3FGL J0700.2+1304@iFÜ¿ôw6@kóæAÀ:6±n¢u
À;œÃT~–?ù?å{Íß@Bs`õ¹*?üഀz¹°¿ïÿ¦´	\u?ïþî j¿Î¿âhµw+ì©¿Ü2qÞrDAGNbcu@´9³Š	PowerLawGB6 J0700+1304?ïþ½Â*R?"ꬔ'Ó¶?$#Ö3'h?"ꬔ'Ó¶?ï'æå°Q?–bçmòS?‹FF—[TN?–bçmòS?ïØÅ!˜è*?g2ÍaçŠ?sonã!?g2ÍaçŠ?ï}‰®\
?|IiÐ.#O?NÝ!xe?|IiÐ.#O?ïû¤ípíd?:™çLËϾ?AlKNžq?:™çLËϾ?ìÏuag4?¿gï×úä?¹‡ìTß_?¿gï×úä?ï´?]õñ?€€Ñ9 ?'ð(z%=°?€€Ñ9 ?ên'MÕS?µl‰³¸ø±?ÆGbȪ±Í?µl‰³¸ø±AGN3FGL J0700.3-6310@q`4óþÀ7	õ`iÍ#À:nߋrÀ;é}ü…!?ÖIÀ'*€÷@pL'8?ÿåÎÿ'r¿ìÃû"­Ãê¿ÎOÀêb×2¿Ô@¿©´Õñ¿çb=üAGNbcu@ªÖ""t¼PowerLawSUMSS J065958-631238?ïä¦h	(É?¬c9"Ó?kY˜/0Ï?¬c9"Ó?ïÁ=Æù¾?‰â®´©'?~?a/ö?‰â®´©'?ïÖ>W'Â?}ѳ,bî?tàԍ«º±?}ѳ,bî?ïßCs"š?PošdCí?p~ÞSD7?PošdCí?ïûe¬W6s?DؔWY?BiN»ãe'?DؔWY?¹â?±)ÆÔ¹uð?¥'4n¾ñå?±)ÆÔ¹uð?ïÒKO<[Ù?|ÁW¢E5?vÚXyßW#?|ÁW¢E5?ïD>Ô?…6EP0ô?—x?·

~?…6EP0ôAGN3FGL J0700.6-6610@qL>_·¼À7¿F uÁMÀ8Á¯bYÀ;"–ÇWB?òâz뮏@ìéÄTXG@ˆì |··¿×zFm!Áq¿â.ƒç^Q"¿áˆYeµ¿åôbèØqAGNbll@"Æ–Ov`PowerLawPKS 0700-661?ïþÒHë3ô?%DÉÂ|@(?"ÛrwÑöã?%DÉÂ|@(?ïoÐbX¹?•¢ˆ¹I#?'ó¶¥ÖÚ?•¢ˆ¹I#?ï¡x£c?†YɾÞ?‡¡þ$Û?†YɾÞ?îhHè{?…Å
Xº?©{q'§¤D?…Å
Xº?ïü¡¼±TT?>Kn`Ì¥?:ò®Zgä?>Kn`Ì¥?ëÎC7[®?ÁÉöِ«?ÀÆó#ΑH?ÁÉöِ«?ï.‡ĸ?—Yꐉ]?š>o&~nñ?—Yꐉ]?éüöòKs?ªÅÎIYO?Ɉ$6Ò5?ªÅÎIYOAGN3FGL J0701.4-4634@p®ŸðË°À1»yß¿î˜À8®àŸ°4À;aš>G?ö—b˜ì@wëb<á@''afÍ?¿âDuÖ¤o"¿äH†¿éuE£'¿¿ïÿ‹TÌ#ôAGNfsrq@8"#ρLogParabolaPKS 0700-465?ï·±ŠÚ—™?'p)¼Dœñ?'Arÿº?'p)¼Dœñ?ï±¥N%j?'€UÛÍÒ?ƒ–¬k	¹"?'€UÛÍÒ?ìý⹞ß?¤d]=@ÿÚ?¸ê4Xûƒ?¤d]=@ÿÚ?ï×ìÕ¶?\	'_3Y?t}
'?\	'_3Y?ïù-³?™°!s׸ð?œpÚJ­±?™°!s׸ð?îUÞa}Q?¶8ù<^®v?ª¢ä»R'?¶8ù<^®v?êS'T¦ h?¯x'^Øø?Ʊº­e~_?¯x'^Øø?ï•Oø»¾?€QI©]ê?Š¬Í âW?€QI©]êAGN3FGL J0702.7-1952@lþ"Àh¡À#j ñÀ9aLF)¯ýÀ;Cä6uÝÓ?ÔcÍ,̚V@…©Îðéb@€ã?ëÓ¿å°p#¿ÐBÜtœ¿à~8iE`¿çb,žª¶´AGNbll@¢Ž6ý!ÿ.PowerLawTXS 0700-197?ïû³"tÎ?A(hö"s5?A1°äÝ@?A(hö"s5?ïŽf3ªk=?—þRj€ÞT?Œfs…øÕ?—þRj€ÞT?ïÔ®ÞØƉ?wÛ!kŽ2?u¨£jïˆ?wÛ!kŽ2?ïÅ>Ce8?X(	þ>[q?}`Þoú?X(	þ>[q?ï挢K‰?k õ¯IM4?isàX5Y?k õ¯IM4?íG¦•*Ÿ?»öšCÁ(‡?µÂËUa-?»öšCÁ(‡?ï#Z‹ogõ?™&n­s?›"®"ÊÏQ?™&n­s?îPĸ£—l?…Nˆú%?ªó´y6%@?…Nˆú%AGN3FGL J0703.4-3914@o;¶m
JÀ-;@Î&iÀ9›Wò/\åÀ;˜ôs®N?ð¹$y\@hó
¤×@M®€0'î¿Þqèa¿äphÈÁ¿ä­™<Ý¿êÂx‹%AGNbcu@'GËƧïžPowerLaw1RXS J070312.7-391417?ïBõÉâô?šË	ø($Ÿ?—¡]ßäi'?šË	ø($Ÿ?îgq~Gƒ¢?¢G¡TN
û?©ˆèôà?¢G¡TN
û?î›å\ÌÅÒ?–̏»y"?¦Aª1{Ôá?–̏»y"?사ùÑ=?ˆõÈpQÍ?»êŸ01v?ˆõÈpQÍ?és@Žh?ŘÚÆga?Ê2ÿíǪ_?ŘÚÆga?à¹ÍN&ÿs?͸Óâ{ñÏ?ތec²?͸Óâ{ñÏ?ሌôo©?À—†ïÈÐ?Üîæ ­õ?À—†ïÈÐ?àè
ÀÎ<?¨´ÿÇ8?ßæ/ê~cˆ?¨´ÿÇ8AGN3FGL J0706.1-4849@p4Ó_ôöÀ1ËóÀVœÅÀ9ob–PÀ;rd­(—?¨	,eÃç@qHA¸1@K¹ÆÄË¿Ý°¨vM±†¿çÖ?#P'¿ä¡‹^ $k¿çzÌìF(AGNbcu@‡m\ú¬ÚPowerLawPMN J0705-4847?ïùug5CY?QôúWèPä?J*bBód"?QôúWèPä?ïÁêöI"?Œ(¸»/Üá?*k¡û?Œ(¸»/Üá?ï½Õë{Ûæ?w‹q_T(•?€Š…"hބ?w‹q_T(•?ïØ}	?VÆv[ ï?sÁ{`úÝ?VÆv[ ï?ï·KæÞEñ?è'N¾í?'-O¥±·?è'N¾í?îq'×û¡n?±_@'Çf?¨æâ€Eé!?±_@'Çf?î1áA£ä?£úÿœû_?¬îïU]·?£úÿœû_?îAè,ϖ×?"0a[_ƒ;?«á}3ây•?"0a[_ƒ;AGN3FGL J0706.5+3744@fo•_x5œ@2ý¾?kOÚÀ9ºgozâÀ;Zˆ
%ð¿òےîÔ @ùó×'ĕ?þ= }Îã¿Øü½¦û=4¿ß£îX_¿àc§wÜ8¿Ñ-3FuҌAGNbll@£™fÂ&€PowerLawGB6 J0706+3744?ïúñÊvõï?>¦ø\ü?D8ÕDô֖?>¦ø\ü?ïԏ/Í?‡˜	æL"r?u¸h)ê?‡˜	æL"r?ïÈxOzš.?w–ñYƒ-ä?{ÃØ5¤eD?w–ñYƒ-ä?ïÿ«‹«çœ>ÿhh±³®{? Žò·>ÿhh±³®{?ïìö¤rÌ·?_R·y%Ë4?c	[¬Ï°p?_R·y%Ë4?ï˕ó¥\?°"ÛËc?žf?ӆy?°"ÛËc?ï‡_>m½·?Œm²QaÍ?Ž(0h.?Œm²QaÍ?ïùÚ`wþ®?H'8æ\0?H–}²ž…<?H'8æ\0AGN3FGL J0707.0+7741@a¦°)(@;H¡€èTÀ8監À;—³%]?èð¬Q}l@ø×è3Û@k_\1¿àd€Ý't¿ß÷ÿ`GéN¿ÞÎö ˆ¿åÆ9¤€AAGNbll@"¸—>«6zPowerLawNVSS J070651+774137?ïÿ§=y»¶>ÿ÷"úá?0©uˆÔæ>ÿ÷"úá?ïØ/¦ƒ.k?~$Ùù83?sè,ˆR®?~$Ùù83?ïí`:IÊF?`fæ'a%?bŸÅÎòê?`fæ'a%?ïßjŸÂ8Û?O³Õ[€"³?pJ°.ÚD?O³Õ[€"³?ïþ¾*âà?"!h¸÷?$¾2á]?"!h¸÷?îÊ,¾œT×?µo"luü?£]4:²Œ?µo"luü?ïâDÛÒ#N?sÛ(ö'o¹?m»$`¶é×?sÛ(ö'o¹?ï}Ÿc:Ày?uK™¸?Lš_¾â?uK™¸AGN3FGL J0707.2+6101@chy?ò^W@9a°,XÀ:aÆÄuÀ;ú'ÌÍ£Œ¿Ü+¹†ã­@`B_A@o Ÿ1ß¿çH©`['¿êB;ԗqv¿áEC#XØ¿ïÿ¤TÕç AGNbll@v8›]PowerLawTXS 0702+612?ïÿ5¥€?–-¬3†?\)Šæ?–-¬3†?ïÐíÐr!?ˆåçQ½ŸÏ?w‰´«U?ˆåçQ½ŸÏ?ï"nÚ±Å?vÀ:)ˆðÃ?‹:¤P2Ɯ?vÀ:)ˆðÃ?ïéß A²?PÕ«%"µ6?f _¦ð£x?PÕ«%"µ6?ïÿ¦ùJüu?
ßÏv—µ^?AºØžÂ>?
ßÏv—µ^?îüÓRwñÿ?®îhÂ¥ñ0? 2Ê؀à?®îhÂ¥ñ0?ï{'<ØùV?Œ>3À—we?¸f˜£@?Œ>3À—we?î±J¸†	?—}"·T
?¤ëT€Ã†h?—}"·T
AGN3FGL J0708.9+2239@hHtÿ†]}@+•³rì‡À9ñÅíhNÀ;²$€€Ä?áo'èƒP@$Êû¼Nz@œ¬_nû`¿"C2jòxi¿à'–6Hø~¿Üa=Yt1ø¿éR6u Ø,AGNbcu@Ÿxú^5?}PowerLawGB6 J0708+2241?ïò>Ù¯‰E?\ˆàÈFó?['L›nì?\ˆàÈFó?ïµ}ü7Ò?Š%
óÆX6?' €ö+;?Š%
óÆX6?ï^ ç'¨?'
üëõó<?";üac<þ?'
üëõó<?ïhýß-;f?jIE*˜æ/?'àDè÷;?jIE*˜æ/?ïÀ}V ~C?}õ¶,QŒ?ÁTtŠÀ?}õ¶,QŒ?íÙ]Ò¡«"?¶XgE¤?±5hÌáß?¶XgE¤?í¼Aûoo?¦÷1–¤<x?²Ýñk‡?¦÷1–¤<x?ìw¦œ%Sæ?›N՚§?¼BËÕ`Î?›N՚§AGN3FGL J0709.7-0256@k4œÆø@ß
ÿÇöÏÀ8JoÛZ.JÀ;³¦‹¤?ÜM$ñ|²@õ(‹k@‰û Iáö¿àÌTw%¦X¿çŒðw]ê¿á5pËL͗¿ç+óÀÎßAGNbll@‹"u\)PowerLawPMN J0709-0255?ïʓ˜è]'?´~]U«	,?z¶3"`["?´~]U«	,?ïµòÞ.t?ñÖcÒÌç?'ƒHf¤Že?ñÖcÒÌç?ﯸ_µû®?‰F‹0žy?"èp?‰F‹0žy?ïüðaZ©? U³?;O^?8|÷ÏJ¶? U³?;O^?ïþ…=ä^†?/DbQ(ýZ?'¬ÚU.4?/DbQ(ýZ?î6͟/°?¸ÊîןÊÇ?¬"&t'/?¸ÊîןÊÇ?ï;6"^Ò?–Ì•ñù"ò?˜™-ye²?–Ì•ñù"ò?ïö$@jíù?Gð°õàP:?S·~«²m÷?Gð°õàP:AGN3FGL J0710.3+5908@c¬|àü.º@9h~_o×À9ržJßÀ;ljÌ&´ ?Àæºòã?‰@ŽfÇ4?ú"—!U<¿ãÌÂó	¿Þ1ãAÙ>J¿ØK«"ÛÙI¿"r¦›N"AGNbll@µiᰉ PowerLaw1H 0658+595?ïþ6ëé6?$ò"úr‰?,'?_
ý?$ò"úr‰?ïÙ|¼¥H‹?ýZd° ?sA¡­[º³?ýZd° ?ïàO)?sÃ/îâÝ?o°æ'E½N?sÃ/îâÝ?ïüª"­em?%5:—ó?:«\«1m,?%5:—ó?ïùõ:Zè?B{83/?H+ûš=?B{83/?îøWN½Êž?±{áH
Ú? z‹×Ó*?±{áH
Ú?ïÆ	&øÅØ?'뉷ŠŠ?|ûl"üì2?'뉷ŠŠ?ïåzH ë?bU½/W?j…¸ú<¨?bU½/WAGN3FGL J0710.5+4732@e8·€4mÆ@6¹Z`ž¦IÀ9mM!À;ÅÉTrH?àÊö8ßx)@ùcãÔP@.0¿æ_p¿åÙLJœ¸¿èR¶ú0:ä¿èhn±í'¿íaœÊrøAGNbll@zýW^ FÇPowerLawS4 0707+47?ïûÏ8"MO?>a¦¥°ÚÚ?@êBA¡?>a¦¥°ÚÚ?ïÌ°Y›õ?~¼O²W?y§ÓJª`?~¼O²W?ï£ÙiNg?|ŠœÝ«?‡	œ¯û:0?|ŠœÝ«?ïqôÛ½3?n›óèý?'܁f@'˜?n›óèý?ïý¾µ™?3º®sÖð?3'	CŠ!?3º®sÖð?îoz	9V?­Y"»¦b??©_o?–?­Y"»¦b??ïš]ƧG?Šæì®v?‰hŽcú^'?Šæì®v?êözh¯t€?¥vœ,Î?Ä&]B.?¥vœ,ÎAGN3FGL J0712.2-6436@q7µ ÝDÀ6*Ð`Ö­À: ²÷8±!À;ÀÀ//˜t¿ûpœ 4=t@£×‹Ê@î¤ûÍ¿Þ{&ëø¿áŠ¡EZ¿æÀ'30ë¿ïÿ§9.8¼AGNbcu@ gÕfÏBPowerLawMRC 0712-643?ïºoŠë	?ƒe­n6¹*?d<!¼»Ï?ƒe­n6¹*?ï˅¨²!Œ?'⿓®g?z=+š¢?'⿓®g?íçèúãe?šwðï6œ?°À¸-J¿V?šwðï6œ?ïÿrdT?
{oÌ$bS?³pr«2Ü?
{oÌ$bS?î恆ÓC^?©vƒ?4?¡—ç\.?©vƒ?4?ï'"'Ÿñ¼?«9ãýE.–?›o²áp?«9ãýE.–?ë,`òšM?°YM؈¿B?ÃN|5–Ëð?°YM؈¿B?ïëΕù7?dB<lk-ã?d1â–Èy?dB<lk-ãAGN3FGL J0712.6+5033@dÖN wm@7Ûß 'áÀ8èpwa`mÀ;‰þÚf"¿Á<¹Ä²L@F›'{@ºÿÅÈw¿à¯âFdF¿ãE4oØ!¿ßÐñ­Šoä¿âa°¤ÊAGNbll@'(ô¼j~úPowerLawGB6 J0712+5033?ïÿÏÉR´>íz¬M"=>ø@†-Ÿt>íz¬M"=?ïݧ¬,]?yì½mTd?q,p¥]z?yì½mTd?ïä`™6·?w€?ëی?kŸf¥!?w€?ëی?ïû¹AÞ$l?' Y'§P"?A÷¡¢N?' Y'§P"?ïÿ®jû»?º
ù¥±n?"\"•…p?º
ù¥±n?ïb
69Î?°°ƒŸØ)?"¾²YŽO?°°ƒŸØ)?ïÂ@«°Œ>?ˆRŽ'T†?~ߪ$ú0î?ˆRŽ'T†?ïÜϸÒ¿?dƒ»€Þ?q˜#҉üv?dƒ»€ÞAGN3FGL J0713.9+1933@hµ«`kz¢@+/¨þ'j÷À8EìòÝÎÀ;=xmži?÷/Oxä@]‰2C@é¨Ì'jP¿Ü	E"¿å]Xë? ¿åð9cy¿èÓ~XHAGNfsrq@€»ÃÉîËûLogParabolaMG2 J071354+1934@?ïü¾)úWþ?6YáÊ°I?:®]AŸ?6YáÊ°I?ïÂ֊¡ë3?~ÝØÃ
?~"ºÅæd?~ÝØÃ
?ﴀòüè?~va'¯"Î?'ßÃ9p"?~va'¯"Î?ïú/ÓF'p?0®éñĐ?G@².µ?0®éñĐ?ïøÇ='?J'
6ܬ?Lã6&U¯?J'
6ܬ?îÊjÒ ?·Ti>i?£^ÉR§?·Ti>i?ïÅÆ{Øq?–Rª];cf?œ'G2<¿Ù?–Rª];cf?ï÷'fÙ]?IžÁ…P~&?Q±3ºOÆ4?IžÁ…P~&AGN3FGL J0718.7-4319@oݝ`˜À+Iä ()À8L· "À:ó>FŒ¬K?óL"=@
 wŒSŠí?ýÜ<ŒAí¿Ñ]n€;N¶¿ØÀ¸æÕ¦T¿Øo'§9À¿Þ7F¢?ŸAAGNbll@¡=($xPowerLawPMN J0718-4319?íwÈl"?³!ßlWY=?·A»Ã,h?³!ßlWY=?á$ù™+-?ÌÎùðïh?ݶÍ©ý¦?ÌÎùðïh?íÖÕ«(ôQ?ŸÁü€?±IR¦¸]v?ŸÁü€?åÇ*Y«ÿ?¨}9j4?ÔqÍ«L¨?¨}9j4?éh Bô$?Â%¼UŸL?Ê_~ô/oã?Â%¼UŸL?¿ñt¨"ª?–Ô@Й?ìÝñjïk?–Ô@Й?ëޟ¶F×?ª)¥©'øû?À…&ä£â?ª)¥©'øû?΄nÔ:?¯jcç,?è^ù¤`
ñ?¯jcç,MIXED3FGL J0719.3+3307@g!A?ÐÐh@3Ú¡–'õÀ7•æLГÀ:õ-Iå&`?ù÷ë|eV@i1kÝɟ?ÿº*áU¿Þ=eÊå
¿âdàé©Q¿ãŸ.×·j¿åqî—YAGNfsrq@€¤Ü(õLogParabolaB2 0716+33?ïýÎZtg?2©…™ƒ?1*þ#Qò?2©…™ƒ?ïÔÑ~Ÿ?'PSë¨´?u—:0ñ?'PSë¨´?ï9Ûì
¼?"´6l$v?˜Íä"6vƒ?"´6l$v?ïõ[  ¹?@@Döï+?UHÀ6/¾?@@Döï+?ïú^	"?DƒÀ0µ"?GƇ"žÚL?DƒÀ0µ"?îÑNGœÝØ?¹5ˆð¹lò?¢ëˆÅ×}?¹5ˆð¹lò?îöÍt¬>?˜öqǧü? –#,$Ø?˜öqǧü?ïñð…ŽŸÀ?U]…†¥Á?\õ=v.Ž?U]…†¥ÁAGN3FGL J0720.0-4010@oƒT`ªdÃÀ(/&Ɖ½À9à¾H¥‹?À;~áxU|3¿Ñ—=7²¸"@l@ÓVq_i¿è^
¾Å¿æáÐæÊû¿ÑžÀ€ÊQ¿ëUS€I€@AGNbcu@œ_Yè>B[PowerLaw1RXS J071939.2-401153?ïâ%Ú/5ù?zõnxKõ±?mÚ%±-Ÿ¡?zõnxKõ±?﵁žl?'Z¯@Mb?'Ÿ¹
¦‹À?'Z¯@Mb?ï?Èb±?JÀrÀI®?˜§Ûß?JÀrÀI®?ïßR݌Qv?XW2Ð7"…?pV'º<ø?XW2Ð7"…?ï£
ê,Õ?áù Ò£?‡<…xl¦±?áù Ò£?íwýdf©O?»®îç)z?´@Þðw?»®îç)z?îZ1ðpž?÷X¦@?ª\àôª"ò?÷X¦@?ʇE?›§Ç•çn ?¦´¿ÁŸ½¸?›§Ç•çn AGN3FGL J0721.4+0404@j–À_k b@!¼@µpÀ97-m "ËÀ;tù»B`Î?à—Ô¹¼`@þeÿ¹3=@:Þ ‰ÍÊ¿ä
ˆ&ªŽ´¿çˆ¬1 ßI¿è_=Ÿ¸4¿ä-²B£AGNfsrq@'…ô>–=ÅPowerLawPMN J0721+0406?ïÿžVþБ?ŽÀ¨ÚW?jCµOj‡?ŽÀ¨ÚW?ï´ÔÑ9Ï?íw´ŽßÏ?'ÊÏIÒX?íw´ŽßÏ?ï×ՠʪ"?s뙂¦Å?t/±X[?s뙂¦Å?ïé`Ž¶É?E]@Ì0±?fŸq@POh?E]@Ì0±?ïþì+? ÑÕÀ½ð?!> ÏYu? ÑÕÀ½ð?îMÇç	äÛ?µœÒù«ŠÚ?«#a²M?µœÒù«ŠÚ?ï®ðƒé·?'عüxԃ?"CßšÖ?'عüxԃ?ï\ñA·ä?f¤ûW?"aÜWɃ?f¤ûWAGN3FGL J0721.9+7120@aÿXÿu–…@<ú€d>nÀ6F#ÿ¹‰#À:XG·N¶F?öˆö#2_#@¥É}·ç?ÿ]g1<û¿ÝX¹ÄK7ѿኸÙáïZ¿à»~úÃr¿ã§LºAGNBLL@{‡[l7aLogParabolaS5 0716+71?ïø÷'r?s·÷m'RW?O¥÷±Ú?s·÷m'RW?ïÕ*8/?ˆ ÿ¥£N_?usüPô†?ˆ ÿ¥£N_?îè,Ql¯+?œ÷O祿b?¡}:æ¡XW?œ÷O祿b?ïÿmù$;?‹.ª°?@Óß[Ôx?‹.ª°?ïó¹ŒÂàT?fäC6bžû?XŒæQá?fäC6bžû?ïóVú7¿?°9Þ–ØF?A•'˜@?°9Þ–ØF?ï(­…§?˜IBôs?šê\è~Ó?˜IBôs?ïÿ'ÿƒð?ÆpÇèW?@4Ë°2§?ÆpÇèWAGN3FGL J0723.2-0728@kæù€õ]æ@Á¶@™MCÀ:Z`·Ð¼FÀ;‹Õ`EK¿ìKÈÀE!j@
	†Nc:b?üÅnA&:ý¿ïX9$câ~?ÃEϯ¢'Ý?´ÿ‹ïj¿Ðï‰ôÆïAGNbcu@»‹_²-PowerLaw1RXS J072259.5-073131?ïþÞâpov?iðO•œu?"×"qSQ?iðO•œu?ïÂDêÚm¹?œÁqmä?~݊³wQ?œÁqmä?ïÛo¯àÙ?nÂé_sR?rH8@ÌÃy?nÂé_sR?ïÿ¸DT˜´>ø0#Ôfá?îßÀ¯Ã›>ø0#Ôfá?ïýêHˆ°?)ƑRÓ Ä?3x¯ÉKŠ¸?)ƑRÓ Ä?îLdŸ¼ÉJ?·u'¹úŽÜ?«9¶ÃÏl?·u'¹úŽÜ?ïǏÐv?|´%/;6J?|rÿ¹w(?|´%/;6J?ïþvÞ-È:?#Dœ'+"?('ôaª?#Dœ'+"AGN3FGL J0723.7+2050@h­O d#–@03ËÿGs\À:Ղ}ô"À;³ÌQ|ÊV?¶ê#A@ËÞ/ ¬ˆ@3i~J‰¿å8'ŽT¹¿ì2ôG"¿ÆàÊv—r3¿ã䂳E‰™AGNbcu@'·€4nPowerLawGB6 J0723+2051?ïÿ¶¿Zð>ûŒ%Ès½X?P>ÿL‰j>ûŒ%Ès½X?ïËá±Fšª?ŠV3ä.d?z'H÷?ŠV3ä.d?ïí­ƒ}Æ?`ÄBúxo?bëR'š-?`ÄBúxo?ïó¡bïA??ÖR)áû?X½:]öâ"??ÖR)áû?ïÿ•AED®?	fùNTQ?
¯žë.Ó?	fùNTQ?]ôŽ?¸@y›?¥Ú#JÓ{?¸@y›?ïÔûóJ?vYTŸ‡vÚ?u'–¤G?vYTŸ‡vÚ?ﺗdn­?tz[4\ê™?Z&þK¾Ó?tz[4\ê™AGN3FGL J0724.1+2857@g² ìt2@3[½ ‡_À9¤LˆnÎëÀ;ÄŸþ7©¿îíPzì°@kDDž:@Ác `Ș¿çíí¸nŠ¼¿æu"—™[©¿äßOᔯû¿ïÿï-mnAGNfsrq@€rL˜_PowerLawGB6 J0723+2859?ïþ¸Þ¿z?@ã€B§m?.$u¯?@ã€B§m?ïØ'Ÿ^Þ?"4àRŃ?sûìN Î?"4àRŃ?ïT¨1ü–-?–8Í7<?•jù»EÐj?–8Í7<?ïÿze&÷?Ž	$T>J?³fá°€?Ž	$T>J?ïÿ—ýãA?ÁBûX¸o?
Žêá²»?ÁBûX¸o?ïFy~œE?§òF\S?—0Ð*Åéh?§òF\S?ï­ø?…ë¿svXó?"ù‡Oõ?…ë¿svXó?ïù‹¯v$Ê?DµJE?IÑBAÐ<¯?DµJEAGN3FGL J0725.2+1425@itXf€@+Õà0VàÀ7Z)¤>8JÀ:æWS£ì?ø|§ÎÕ@9ðh2n@ø45f¿'¿á,H›Ó¿ãàNŒ€–¿äXɒ°œ@¿åµØ[4AGNFSRQ@z³	€²BLogParabola4C +14.23?ïý•{
"¹?5±d+>?3T(©Êò¶?5±d+>?ïÐÕ0.Ø?…IÍBWWD?wöKÜ?…IÍBWWD?ï_Bº9Í?'¿‰aJð*?"7§ø]?'¿‰aJð*?ïÿ¹«A¡>òɉ¾½lÉ?•#
/ÚZ>òɉ¾½lÉ?ïûO)?G½Ø'¿?BÃ\Oii¨?G½Ø'¿?î•30·‹{?»&Jð
-?¦¬ÌøÒËP?»&Jð
-?ï-IüÅ°E?–Æ{ß»?šVÀlqaO?–Æ{ß»?ïÿϜ=–l>ùu±åTš
>ø1üšËF>ùu±åTš
AGN3FGL J0725.8-0054@k69Àëíú@òÆÖ¤èÀ9EG1í¹À;kÛ._"?»ÍÌçyÌJ@%–¸Öq@'-ÈÈ0¿ä(›	—j¿äŠÔ˯ýo¿Ù+²ÔÍ]¿âr»7½ËAAGNbcu@—	1Þi­CPowerLawPKS 0723-008?ïýO~ñ?*ԁ"Ïè?5"
cÏô‹?*ԁ"Ïè?ï«?Ž¶;¼?"ÍJUvšŠ?…0`/€ü?"ÍJUvšŠ?ïÕÍo''?r)³15!3?uH™©¸?r)³15!3?ïÓ+/G…?ZëTüùf¼?vjh@ª]?ZëTüùf¼?ïù½FO£4?C³†ÔÛ&'?I
æëÇù`?C³†ÔÛ&'?íÏN=G+?¹Ñzq
YJ?±‡U_¡)?¹Ñzq
YJ?ï˜[ÎÝÉ?‹U•ÊgÜ?‰é:ÏHx?‹U•ÊgÜ?îj×ty¶?•I,nÈà"?©R‡–§?•I,nÈà"AGN3FGL J0726.6-4727@p6B 6mÀ,;ý!(n´À8Æ¡ëw²¿À;TwÓv4:?ðMó=yÞ@"rYä¢×@¶- t"§¿â¿:pœÔ¿æÃÅð˜7¿çù=TZ†¿îK7ÛRelAGNfsrq@…P[ô‡ü¹PowerLawPMN J0726-4728?ïðÝ(è?WÊ¿ºÁ6?_èF*$Ïj?WÊ¿ºÁ6?îÌþ"=?¥/^ë²eú?£0ºãÓ?¥/^ë²eú?ïL?…!Aù\"M?–n¤\"v?…!Aù\"M?ìëµg¢Èå?§é1•ù?¸¢TÄ3"Y?§é1•ù?ïæ	`ô.?j˜½Ÿ÷?iöŸ
1Ðâ?j˜½Ÿ÷?åAz™×µ'?Ë0‰hQ«¢?Õ}
ÌP"Ý?Ë0‰hQ«¢?î©in¿·w?š;½Í(ÝÝ?¥iiào"?š;½Í(ÝÝ?ᦚ··øæ?±»ßwpæ!?ܲʐ3?±»ßwpæ!AGN3FGL J0728.0+4828@e2;o@9ÍÕߛªÀ:‹"äþòºÀ;çú#G-¿ú›yhKÃÎ@ÒÍ`Æ@÷ýÀ4¸ï¿êÞÜKðÄN¿à§ê{ož¿ÝDTî™Ñ¿ê<ߕ:AGNbcu@"ZÇâ'@¸PowerLawGB6 J0727+4827?ïá÷ÁÃu?lÊçJ¡–Ã?n>ãBý?lÊçJ¡–Ã?ïÛggBYl?ƒÕAӍj?rLLi"?ƒÕAӍj?ï$Vß4ÙQ?¦$n(ºz?›u$!ûÛâ?¦$n(ºz?ïÿ®Íø	Ö>û³hÁjz?L?œÓ>û³hÁjz?ïaÈ=à¥?"Ȑ˜÷°?"ÆøL'dŸ?"Ȑ˜÷°?ï3ëÈn ø?ªyìBBv›?™'†ë\¨ú?ªyìBBv›?í`ZJú$I?§îzÅ¿$?´ý-¨œÑ8?§îzÅ¿$?ï÷Λâ|À?P_¬‡Ó?PbÇëO?P_¬‡ÓAGN3FGL J0729.5-3127@n¢å>‰©Àŵ ÝDÀ9´I窞¥À;Q¸Æ…Šï¿ë=iöqi'@–'%†ø,@;µ¿j
»¿ãô§¾6-¿êˆØ‰C‹¿í
ÎÖü¿~ǁfûjMAGNbcu@ƒ#ýVlôPowerLawNVSS J072922-313128?ïüͱËO?>¾%Ï®Œ?9'r¤~šs?>¾%Ï®Œ?ï¸ßV߂)?Ž6ep0å\?È*W=½É?Ž6ep0å\?ïvÔXîj?…ª5í»ø?Œ"JæTɋ?…ª5í»ø?ïÿÅÌ8¹k>ò( å@|s>ýÑجxH>ò( å@|s?ïê¥oˆŽ?f꿛õ¶?eZ®ß2?f꿛õ¶?íï`MÑ!Ï?¼yÇÊ·ý;?°"ý'R؉?¼yÇÊ·ý;?îÞTÕM™?—ŧsß¼7?¢²¬ç´m?—ŧsß¼7?ïù°‡`ÿ?JõOÿf/1?I?ú¢Ye&?JõOÿf/1AGN3FGL J0729.7-1448@lÍòà\̊?øb½ßôò±À9¾hêÀ;[Sã¬ã?ÖeäJþè@ÜÕô=Ôø@\›`C™¿à±ùĞøK¿èÄxãáo¿ç¿ûö¹Ž¿×L¤•ÃPSRPSR@'Ç+JPowerLawPSR J0729-1448?ïü·@s–?^¤í)Íz?:EýCà2~?^¤í)Íz?ïoa«.u?ªVº4º^ñ?'ßʚ1^?ªVº4º^ñ?ïoXg3?ˆ}HÔOæ?'TüS¥?ˆ}HÔOæ?喝÷
–?ióP]P?…'ÂNˆh?ióP]P?ïå{<aZ8?r$/ê¾LD?j"Ù&h?r$/ê¾LD?êúW­n–>?ċH¯,?Ä¡JE§?ċH¯,?íñü®U­?£Ø/3LÈ+?°pŒä£…?£Ø/3LÈ+?ëàüŖ€=?±«^g9V*?À|é¥ÿ?±«^g9V*AGN3FGL J0730.2-1141@lxl_9K{@	Ø_ÒùbÀ6b²<'ÎÀ:l)±ª1—?ø'{j×@m^ÒsTá@¸Æ§Þ¿áapD­üJ¿äǜԷ|Ù¿äç|×I±¿æ£#$a"AGNfsrq@vï'å!WiLogParabolaPKS 0727-11?ï÷Ï4[&l?X;qVj¬?Pa—=áL<?X;qVj¬?ï"D׺*x?¢AŸ©öU?ŠîÊ
–*%?¢AŸ©öU?îÉE5>P?œ+Y.¡Qj?£n+ªeÿ?œ+Y.¡Qj?ïû•âÈ7?0+úœÎ3S?A«å[ÄãÔ?0+úœÎ3S?ïñ–1¸½?_I±*ÙC?]ÌÓD˜…Ò?_I±*ÙC?í%é'¯•?Â\ë8ÙÌ?¶Ð·.DØ?Â\ë8ÙÌ?îv$¬Ý™#? Dý:Å?¨µ0nŸÕ? Dý:Å?ïúÉó‡)]?AÊ!kì£?DØ2f2 ?AÊ!kì£AGN3FGL J0730.3+6720@b'ºKâ@<™åàš	+À:Xg`ai§À;þÓôß:Ž¿â<žüÚ܅@¤­'ÊÈf@ëø :G¥¿éÆB+ôz'¿äòíVkWοèˆ(»`å¿ïÿl³Ì9™AGNfsrq@ƒéL~($PowerLawGB6 J0731+6718?ï÷Ô]ùÃ?NCº3˜NR?PWFfŠ6!?NCº3˜NR?ïߎñJ±?xn|oE<à?p8‡>ÐÛ²?xn|oE<à?ï=vPœÙ?ˆä-øœðw?˜Q5ïÔxc?ˆä-øœðw?ïòp§KÍ£?Eòú{"¥Ö?[°ì²Ëc?Eòú{"¥Ö?ïó9gÍ6?\ËH{4wÙ?Y0
锅?\ËH{4wÙ?ï/ÓúŠí?®Â¡7¹"ù?œÚ€®¢Q?®Â¡7¹"ù?îTp¼øæ©? ÛÞ,ƒ‡-?ª¸ô3Jt? ÛÞ,ƒ‡-?îυZTW?–Fèò@î?£¯«6¡"?–Fèò@îAGN3FGL J0730.5+3307@g;öÿ:Þ"@6e>‰©À9ù>
ÈÂÀ;̐"£¶¿îvº8—îk@2ˆá:˜@ïý |¢=?ÍØ¢òŽ0¿è䴲Ϡ'¿ßÆNdMBº¿ÓŒÓ
‡ #AGNbll@FޞšPowerLaw1RXS J073026.0+330727?ïÿdÈ	L8?j ¯M?fù!qÖ?j ¯M?ïÚԚÕ"?j.dôέ?r•²¬'¢D?j.dôέ?ïã¤Á¯§?iã-{×?l[>tÞä?iã-{×?ïÿnßuŠµ?¶rbÍ&?$"¹DF?¶rbÍ&?ïÿ¬t<¾?ά¼²0"?ênׁ—?ά¼²0"?ï%ýÛì%?®j¡¶(™?›@D'»f?®j¡¶(™?ï׃ӚØo?v§äy&ˆ†?t>è'?v§äy&ˆ†?ïöÝwÈl?N{ÿj¨{?REÚ["E?N{ÿj¨{AGN3FGL J0730.5-0537@kÍóFí$@C·À AÀ9ÃÁð8À;Šf¿àîð…†	@Ä:ø‰@Í쟥ø"¿æSñÜѧ¨¿ä´Ä16ž¿ÅÇ$%hA¿êèˆ±ò´AGNbcu@¢_6âëPowerLawTXS 0728-054?ïåŒ[ú/?g3õߘg?js恩¸Ì?g3õߘg?ï¶Ê& Èo?ŸºKê?'Mvr¦zN?ŸºKê?îýü¡ê?•"¦
OÁ?  5ðè`?•"¦
OÁ?ïù`™üH™?6֛•j??J}—Z‹¶™?6֛•j??žú¬"?Œ=,cé¼û?Ž˜K£²ñ?Œ=,cé¼û?î*¿Ôäì?¹kaÀíÏ?­TR±±F?¹kaÀíÏ?íX^KÃV?¥×:¦ÿd£?µ?ÅØÓ?¥×:¦ÿd£?ïÂÿüÏôÊ?u¤n€,ˆd?~€°Âʧ?u¤n€,ˆdAGN3FGL J0730.5-6606@qZhŸÆÚEÀ4Õ  0øÀ9ÑwÛðuÀ;‡±ñ\Ï¿ï;¹ñöw@
»7
³Fê?ü 4á368¿éÇO á¿Ø´–×ꯃ¿Á! ]FñÆ¿Ý8úÉpˆAGNbcu@²•]à
qPowerLawPMN J0730-6602?ïû';&F¼?dÿ†2"?A»2MðM?dÿ†2"?ï̄)9?Š ]ºè–#?y½ó¡½÷g?Š ]ºè–#?ïâ?#Æž?g•«HŠŠ?mÀÜ5ÃÙÑ?g•«HŠŠ?ïÿiљ©ù?
bKCÔ?ÅÍ«
µ'?
bKCÔ?ïô§Aç›?\pkäÞÉ?Wè±~Û?\pkäÞÉ?îéíj¸@à?°~c¿4aE?¡a)T{ò?°~c¿4aE?ïÒ/}¤¤?z#Ê­á@Ì?vèAG2?z#Ê­á@Ì?ïúvô>^?A"»˜Ga?F'è\§¼‡?A"»˜GaAGN3FGL J0732.2-4638@p0Ã?…Q
À)ÌG¢'vÀ9e¾/áoÀ;làæ_E
?úÜÐ*zR@šWÍ|2@)ë‰%ƒ¿Ø8qÂKOÆ¿æ¶É ûì(¿îýØP
´t¿ïýïmqٝAGNbcu@'Åá@N¥LogParabolaPKS 0731-465?ïaß5kX?£4U@P'?"ÜÄs]
?£4U@P'?àŸHØêoþ?Ì%Ö7sxŒ?ÞÁnN+ ?Ì%Ö7sxŒ?軯ü¼ÿ?±'ÏҎùE?ÍA¼
?±'ÏҎùE?ã˜ö£'H?­<"c‡_?Øθûoß?­<"c‡_?ï	Ñóí?¬ 6Œq"?žÞ>
èì\?¬ 6Œq"?Â*H*[|?Ç^G§/?ëumù5i!?Ç^G§/?ê5‹l%?±•U؝½?Ç+­ÒO‡l?±•U؝½?ÅÁbáª?®ÿë§ì3>?ꏸûgG•?®ÿë§ì3>MIXED3FGL J0733.5+5153@dÀm ‹]@;Vš ¨4À:pÚ7›À;×5Ú­` ¿ÏÐqûxf@
dÈÚ#øX?ûÚß?ãýb"Rf?èòKÅXí¶¿ã¬[ñ"׿½7'lÃf‹AGNbcu@¶ß£¼ÓZ†PowerLawNVSS J073326+515355?ïþÅœ€¡? ÁÈ_Æc?#®dDÈJ…? ÁÈ_Æc?ï×Ç`ý?£q_ð?tqœBrî˜?£q_ð?ïÓo$^>?rùzòÞæ?vHn€,Ý?rùzòÞæ?ïú( 2:?8ˆô‡äf?G]'¡4?8ˆô‡äf?ïû°±ItÏ?A{€Î.?A=;†ÌU+?A{€Î.?ïýy+Ô´?²ò`X
ç?žàPÕ]ÿŠ?²ò`X
ç?ï¡£È`pG?ˆûÒï?‡—
á¶J?ˆûÒï?ïÀÁ=níÁ?{Ö´W5?ŸaDi—˜?{Ö´W5AGN3FGL J0733.8+5021@döè ÓI¿@;½°ŸpÀ9Å»{k±)À;Òîî_Č¿ñ§fiœ@îKAFò-@¾ÿ¯£¿çúÚâµû¿æª¢_)Êî¿çCÑ`&Ó¡¿ã-ËÏAGNfsrq@†Op#̎PowerLawTXS 0730+504?ïÿç±!>åÞ®ŠŽ,2>èNÍ1¸
>åÞ®ŠŽ,2?ïÙúͧŒ?ƒ"cØn¢ê?s™(z?ƒ"cØn¢ê?ïëª_(sU?a[ë9G?dU ãëBs?a[ë9G?ïÿë3Ùåÿ>×!Ö<dŸ»>äÌQkÄfG>×!Ö<dŸ»?ïÿÜþŒý>óC1ßRª°>ñ€ÁÒŸŒ>óC1ßRª°?ïZ
j'?¨jà€µ|?"¾²¯tŠ1?¨jà€µ|?ïèë+æ|?fµæ½Ìò<?gÓå°tƒ?fµæ½Ìò<?ïþËBð%Ô? éqP(Ò&?#KÍIÛYJ? éqP(Ò&AGN3FGL J0733.8+4108@f7)à¤&@9
ohیÀ:.ήN\"À;ê‹y¢ƒ? ¨8t¹Ûñ@
(2F#Oæ@ÆÎ`u¶¿ì˜î
V'€¿Íɉ¬¿–¿áf`­G~ø¿×¶óËØõ¿AGNbll@—$*™0¾PowerLawGB6 J0733+4111?ïþ}úµEû?'âlžz	?( Wú@
 ?'âlžz	?ïԕ".ÿ%?…)1'ú7!?uµ5òÏA¦?…)1'ú7!?ïÓÂÎ=³?tŒ•rÈû?vz¹Ýf?tŒ•rÈû?ïãVª9W˜?Sa¢*Ž~?l©Uúâw˜?Sa¢*Ž~?ïûŸ¾KՖ?=XWt¿^¯?A¼R\¯?=XWt¿^¯?îÌXÑ'zm?°	Ñtñ&p?£:rï@'(?°	Ñtñ&p?dV´?‰`v}S?Š]¦ìkã#?‰`v}S?î€Ð¼èË}?™éQНµà?§òô3+'?™éQНµàAGN3FGL J0734.3-7709@rŽ¿ìºÀ8(àÉÙÓÀ8аô)2À;n`TÔn?é"tþžoÜ@H50cu@R'ıJ¿Õâ°)åù¿æHû*‹¿åðûDU¿çq$Ê(œpAGNbcu@Š{IQ'ªPowerLawPKS 0736-770?ïþ‡
¿ ?(kók–I?' A,Ø?(kók–I?ï±b³©e??"m®ír'?ƒ§SLT?"m®ír'?ï©RJêMÖ?'ÊԘ©Ë?…«mO»^x?'ÊԘ©Ë?ﱎ¨ÿ?a¢ŽÞö20?ƒœ&w 7?a¢ŽÞö20?ïû@'¸UÇ?HÝ欓Z×?Bÿa%A¼?HÝ欓Z×?îqÀ"°%Í?°«ÛÂÊD¦?¨ãö´ý£.?°«ÛÂÊD¦?ï#âH?–>"ðß?›@GaÌ?–>"ðß?îLù³×!?'Ÿ³ <1E?«0oEžtê?'Ÿ³ <1EAGN3FGL J0734.7-1558@mž@ÈG,@ž 'ðÙÀ7⥤i×4À:÷ì^òÕ@™ãC0×8@²ß¢<€d@"fx/º¿ÖÒXbËt¿ãAVÊŔ'¿è%n+¬¬¿íì¹®€PSRPSR@†]ÔɅðoPLExpCutoffLAT PSR J0734-1559?0À·'Y­á?=ÆneR?§?ïýçéL¤?=ÆneR?§?£Öâ=M?Àa 0•?î'×ЮP?Àa 0•?®LÁT¦¸?¡#Ècü?î3ꊚE?¡#Ècü?eEµþìe?P$''^µ?ïêºJ-›?P$''^µ?6_ÁaëYF?26Tpv[?ïý4»Ø€?26Tpv[?(™}õ6>?¯ôĕI<…?ï‹]™ì®G?¯ôĕI<…?¼HÓÕì?‡Ô˜.p¼è?ïR✠?‡Ô˜.p¼è?)ŒÇ)£²í?Mló8?ïþg3À̹?Mló8PSR3FGL J0738.1+1741@i;dÀßXÁ@2'ŸªTÓÀ7"^™éJ²À:ÅD1ˆ8H?äëWÒNí@yéØ÷'"@
?·¥ô¿Ü3†Ç¿áÏ-à8¿Þñë²7—"¿Ü»ã"$VAGNbll@'v{J#9ÁPowerLawPKS 0735+17?ïÿ®'>ý0ÙbñŠœ?áÿ¨>ý0ÙbñŠœ?ï˝ˆøÇ?‡aôØ'ˀ?z1;hä(Š?‡aôØ'ˀ?ïæGXóÐá?pk6¢Xûß?i¸§Dˆ¶??pk6¢Xûß?ïä
C	"ÿ?SNÆÓ¶»[?kò¼î+ðà?SNÆÓ¶»[?ïÿ¼US?)Y¡€þ?ˆn1Œ™?)Y¡€þ?îç¯ñ—)?²jY[£?¡ŽuÂtp?²jY[£?ïÏ»bþ8?"€|÷~O‡?xq"M!ä?"€|÷~O‡?ï|8EÒÙ?ƒAUȳ?lXümÑ?ƒAUȳAGN3FGL J0739.4+0137@kËßÒc@&е~ÒmöÀ8%W¨]'À;T»ÉoJ;?û$G%Ž@>«6z@ SMÚÔL¿á𗳡"Ê¿è\·€à:=¿çËíSÕë¿ìÆ©C'ŒAGNfsrq@tpû~ÿ—LogParabolaPKS 0736+01?ï̎=ðÑd?tGâ ×Ë?y¸àöiB(?tGâ ×Ë?ïws‡"½?¥Öu£?Ÿˆ.0l?¥Öu£?îYa9o§?œÍau¥np?ªiìj½\C?œÍau¥np?íÞ(+,Ú?Ž›Æ'h»?±¾¦"¾µ?Ž›Æ'h»?ï">Nq±?†'K‡ñ?‹03BËÍ?†'K‡ñ?ë¯XˆµÏ8?Á͎úÀa@?ÁBÝ(à ?Á͎úÀa@?íÐ#¬?¡z;œ˜t?±?ï¤Ö?¡z;œ˜t?é©DúÛÓÑ?²'-Õ/Û?ÉZ쐰½?²'-Õ/ÛAGN3FGL J0740.8+6621@b¶°À&Ì@=œzߚ.ëÀ:frû À<Àu¦uJ?õ»½ ´ëÛ@7[íçy¡@1Ø@žUÁ¿æ]¢ÿ/0Ö¿Ñ~"´Ç6O¿æ½"e¹ú¿ïÿïÝÚ!…PSRPSR@"<ÓZ…ˆPowerLawPSR J0742+6620?áϔ—?Ðïý3FÿC?Ýø`ÖÑÕÃ?Ðïý3FÿC?Ú¶ñê?Ëï=mÉ?âÀ$‡7±?Ëï=mÉ?æíÚ|@uï?²å™=du²?Ò$K!?²å™=du²?ßë!Z²lé?©fqˊ²•?à
oR¦ÉŒ?©fqˊ²•?×±>>² Ú?Ï@yF+Í'?ä'`য"?Ï@yF+Í'?Â×Bñ"Ø?Å{Eü8 0?ëJ/{ÚÊ?Å{Eü8 0?Ö¬vêÜÇ?º´*$ÒÙg?ä©ÄŠ'œ~?º´*$ÒÙg?·a£<?"=ø–Ñ©†?í3ÎtÓÎ?"=ø–Ñ©†MIXED3FGL J0742.4-8133c@r]…À3aVÀ8ù_{šÀ:ÃÃX¯Ä~À;»‰'ä™r¿°º"ËZ…@	Ü=IaÕ?÷l?¸ý¿ì‡/ÆäwܿٓtvŸn›¿àÁM<ɵ?Ø2E-¹AGNbcu@ÒL°Ä›¥ãPowerLawSUMSS J074220-813139 ?ïü§F'›?8;házqX?:ÅËT^•?8;házqX?ïƖ;ã}`?'›Cøzû?|´áî¤èG?'›Cøzû?ï|;×¾å¦?Žï ¸	Ó?x…
Jµ>?Žï ¸	Ó?ïý×5`\?&ó(VY?1FWç|õß?&ó(VY?ïùä
?LE"'?IÁÄoB]Ú?LE"'?îêj™Pô?´os"ò÷Ì?¡X	Yڌµ?´os"ò÷Ì?ïž\«k?‰™N?ˆ}8/´]?‰™N?ïÖ. =§?wBW'ë‡?túhô´ƒ?wBW'ë‡AGN3FGL J0742.6+5444@dam¿‹›ª@=Œ`Ëò²À7ÅÐÂû'³À;3ÁÑÇ'?÷¿n2†@È8'ŸT@(ªªŽ—¿áV£Ðª'¿ãôIL
€É¿äŸ&ãæç"¿èU)ßÕòAGNfsrq@|¢ŒL˜_LogParabolaGB6 J0742+5444?ïüH©‰s?C±
8'G??e¸ÔQO¾?C±
8'G?ïÞ2"ƒ³‡?€[øÀï1?pæ¶!ùp¸?€[øÀï1?ïÃÃä›Ëx?x+õŸÿb??~
¿Ø³æ?x+õŸÿb??ïÿœ!«˜Â>ús7oÆ?÷›–ƒO]>ús7oÆ?ïöwª9-?VI3‰¨?SÝ'œ§m?VI3‰¨?ïA"?°?²MÊ%b?½×Ö/ý?²MÊ%b?îõrԚã?™ÙZKØ=? ¨Ò¸óFÌ?™ÙZKØ=?ïÿ¶Côü?³ÖÎeœ?o4uŒæ³?³ÖÎeœAGN3FGL J0742.6-5623@pÍN wmÀ/c1àLÜRÀ9Ëú/ÜfžÀ;£'ð	è·?ãmÛç-1x@7º¢Rв@n[à¦sr¿èV€G솿âM.6c¿ïþœ ::¿îŒxϨ'AGNfsrq@{×>«6zPowerLawPMN J0743-5619?îˆ<u.ÞÃ?­F7÷¨?§|8®ÉáÉ?­F7÷¨?ï*š¢
ì?˜¬*a:s?š¬«Á¥¬k?˜¬*a:s?îQ°ˆÖ?šM…m2uƒ?®äù7š?šM…m2uƒ?íkÝQæbÜ?wUÛU†?´¡q:ܞ?wUÛU†?è¬÷QõZ?ÇEœª£µ°?ÍO¨"¸*˜?ÇEœª£µ°?ãŽÝÖÏ?Ñ/(õË&b?ØãÒDRaÄ?Ñ/(õË&b?êƒ×w9Œ-?¯¸xðÁCŽ?Åð¢#ÏN?¯¸xðÁCŽ?ØiÞÜÕê"?´¨]ƒã?ãË'•
¶?´¨]ƒãMIXED3FGL J0742.7-2824@ny)Ÿ¡—ÀÎE s'•À8àa'ÑÖøÀ;!º+àX›?ö¯þr·,§@C1.ãÃ@íèô>׿Ò&'Z¶°¿äíî/ýW¿êàŧ‹í¿ïL3íÙPSRPSR@"­`"&þPLExpCutoffPSR J0742-2822?ޜ?ðʜ¶?ÉÉ/û+–?à±àš±¥?ÉÉ/û+–?Á`á®Ó‰ø?Ã~"J'™?ë§Ç"K'?Ã~"J'™?å/ìñt;?´nuIê?Ôý &Š?´nuIê?Ø[üÊ/Rm?¥.N܁ף?ãÒšèVÊ?¥.N܁ף?±þ'š£ƒ?±Ë$ 7Ÿ?íÀ-̹N?±Ë$ 7Ÿ?™WH0¡?¬ûµ¥$º?ï5GçºS?¬ûµ¥$º?Èæ(±'¢?µAzߧí?éÆuӟW|?µAzߧí?«Xë"ª"I?šEG$/I?îJqMþ™+?šEG$/IMIXED3FGL J0744.1-3804@oŒ-@ªêûÀçÆ«±ÊÀ9®œ­JP†À;@R,†q¿£Ì0ú&@
m‡Aþ'@q³?ˆ?¿ç¼d™Ì¿æÐ9Ó$C›¿ë3@ð=ÈÁ¿ïÿ+‰/OAGNbcu@}©	þ†ƒ<PowerLawPMN J0743-3804?ï¢Æ•"ëú?'üÌ@vAð?‡NZv-¤?'üÌ@vAð?ïg¢¨$æƒ? Îš$«qc?"«Š™•? Îš$«qc?î%cî"C2?˜]¼rgC?­©ÁHâ?˜]¼rgC?ï34‹U'µ?€y/lÛE?™™nŽn'Z?€y/lÛE?íó€Úñ?´DD™æ?°cÿÒZˆ?´DD™æ?çѦú'gW?ˤa¯Ùˆ?Ð\²
Ý1R?ˤa¯Ùˆ?ì6â\®W?¨;†=Aþ?¾Hï]J?¨;†=Aþ?ä)Ëökµ?¹µ®yÚÊ?×­Äh(–?¹µ®yÚÊAGN3FGL J0744.3+7434@aˆÏÃø@=–²ß»¼ÚÀ9Êìˆ3@À;Ô=ß^ŸÉ?ًž`Ë\@Ú6n&#U?ÿÉ¾Ð_Ô¿æ
ÂmDÉU¿è¿²sð‡¿Ñ]i4'пƧrŒ¤AGNbll@¢²ÅF
¦LPowerLawMS 0737.9+7441?ïÿ$ê‰æ?
wGfÅÁx?öµa•Aº?
wGfÅÁx?ïÝRQ965?~Çiàh:õ?qV×VVa€?~Çiàh:õ?ïòºæ¬ƒ?nqÎÿÍð)?ZŠ2Ýóœ¸?nqÎÿÍð)?ïùg™†B?3
ƒÈqç?JašO"?3
ƒÈqç?ïÿ|¼-7?§úkJ?ht/òt?§úkJ?ï9Dš8Ñ?²võšØP<?žø×s˜Ü?²võšØP<?ïòÒâÝÒ¦?i:ŠýãÝÃ?ZZ9áeô›?i:ŠýãÝÃ?ïÜz¿0Nt?fY×׫ij?q {Ɓý?fY×׫ijAGN3FGL J0744.8-4028@oÑÞß)À 	ÙÀ%I'À9cý!(n´À;RZ8Zº?åä68@
h/žÿ	5@·[à{€T¿èø-®d¿Õ^Ž1퟿äC†Änž2¿ïÿž'ƒ© AGNbcu@­yõY³ÐPowerLawPMN J0744-4032?à1<{¹èL?ÐeÒéá?ߝ‡Œ/h?ÐeÒéá?èàɽ4?Äö@ó?̸Ù/Å?Äö@ó?æ¢DÛH²ï?²¯PS;½?Ò»vInš#?²¯PS;½?èØ7?¡ä;·Ýc?ÍÀŸ#鋗?¡ä;·Ýc?¼Rh$#T?Át†Ò9Á?ìu²û{?Át†Ò9Á?É3R—t ?Èø:õÛu?é³+Z:¢Ø?Èø:õÛu?Ú3Q
ð?¾·M–ƒ1?âæp×zó?¾·M–ƒ1?Ê°€c#?«hÉ{¶9?é|þç7?«hÉ{¶9MIXED3FGL J0746.4+2540@hWFà!q@6Ø1ôoÀ9MC%¾=À;¨¤Ô`?¿ô¨cpŒ@üç¨eÝ@¶šà@œþ¿èÎíd?οêß"Œ"Dè¿çO¢D
 ¿ïÿû
LàAGNfsrq@r¿Ö"uPowerLawB2 0743+25?ïÿ;Òò‰S?¸âœþ¥´?…¡¸'ª?¸âœþ¥´?ïØc'm'?†KqËýÍ?sÎ@Pæ??†KqËýÍ?ï[xÔ²°?'Ûôs_@?"ðB?ø?'Ûôs_@?ïÿ~¤ºxÑ?Kµ´^¨Ô?+q	表?Kµ´^¨Ô?ïÿ‹öî´S?
tw¾?
5^Ûí?
tw¾?ï'êÕìR?±çž"ï?›¥[J§º?±çž"ï?ï±EkÞº$?ƒg·'/š[?ƒ®¤ø+M?ƒg·'/š[?ïôësùCp?QߒóõG ?V)15]?QߒóõG AGN3FGL J0746.6-0706@l6Èó#@!½•`$À9þ!ã–¹À;kfKŽt?Õ:[¬ñ@ºÁeæcÍ@‡Â yÒ?ïìkü'ƒR¿å›Üc‡}§¿â÷ˆ"¢Ø¿êøÈ¥î(AGNbcu@¡žÃä%®æPowerLawPMN J0746-0709?ïøP
{ÑT?Je ¸?N¿ÕÁ?Je ¸?ï¢YJÜ'?wÑÛU(?‡i­R:Ù?wÑÛU(?£öóE?™nñ»žÆ?¥·¥¾Øý¹?™nñ»žÆ?ï›Ótþüí?k›«Þ½Õ?‰"µñðÇ?k›«Þ½Õ?ïçSïžçj?q®AúÔЅ?h¬D;ÞC?q®AúÔЅ?í¢ûSâš?½÷ê·W|?²è%b¢ýê?½÷ê·W|?í UWö6(?¥‡w¢á²[?¶ýU?à[C?¥‡w¢á²[?ík´ÐSP?œ˜%äǗ?´¢[ƒ53{?œ˜%äǗAGN3FGL J0746.6-4756@pUÕ`"¥À&¢ù;.ªÀ8øžâ®¶aÀ;Wƒï
iu?æüEH3 k@x¡Ú±@¾_쥿ç®(&ÃA¿äãˬfOë¿á%]èÇî¿ÖM¹º1¦AGNbcu@–»'»/ìPowerLawPMN J0746-4755?ïü©ü4»Á?6x?ÜêXã?:°[k??6x?ÜêXã?ï¤lÔ>±?'r±"d+¸?†äÊþ*?'r±"d+¸?ïâþ*Æ[?pGI]ço?màÜÝ+?pGI]ço?ïÈWŸE¢?\=KâD?~;Ô8œ>¾?\=KâD?ïöjyØÿ?Vp…0Nyý?S+"	ñ˜?Vp…0Nyý?í›°â?¾xämRi?·Û'<ž°Ÿ?¾xämRi?ï*ᇟ¥?•°¿$?š£Ý©ä¡r?•°¿$?î|'uåµQ?'®Ñýҝ?¨=ˆ¢€'î?'®ÑýҝAGN3FGL J0746.9+8511@`à·ö@<. Eð¥À:/(âwYÀ;ÐÍ×°VÀaK:»è¤@ïàÚñ?ü˜ì€Fac¿é™'Xßj3¿à&ÀøÇì¿Ö8ðÐÞg¿ÍÅaðA¶AGNbcu@²(Ý/Ÿ¾PowerLawNVSS J074715+851208?ïÿ×z"Š?y WC·?µ{Ï?y WC·?ïâJ'ôï3?~ÖðZy?mµØ?JÜ[?~ÖðZy?ïçQÀ¼ô?V'Ú§Y'?h®?
r•?V'Ú§Y'?ïÿþÚTäx>žwõ­_Cã>¢YðâPk >žwõ­_Cã?ïýÉÇQ?,C›;´+¶?1±Æˆ·ô?,C›;´+¶?ïP]Ì ?³
4ýgé+?ÕôAD"º?³
4ýgé+?ïØ=§¼ƒ:?uéۅ]1?sá,QGB?uéۅ]1?ïÿØ:ǯµ>ýo¶0l=>óâ"2øž>ýo¶0l=AGN3FGL J0747.2-3311@o
•$ÝÀٟîó=À8ƒjƒ+™À:Ø G2Ä?Î,Ùx'ôö@S­|$"@y¹h¿â50hJ
¸¿æNíìW+¶¿å)‡ZID¿ä…R\Ä&5AGNbcu@‰×z–¼PowerLawPKS 0745-330?ïÿ"zSXB?òEâ.ç»?°¸òü+
?òEâ.ç»?ï¦|òy?œ
r;þ?†`ßõ»±Ü?œ
r;þ?ïÍh8M¤N?yJ7Àà?yKãß]%$?yJ7Àà?ïý>>T$? ß|'ѱ'?7þ2Á	m? ß|'ѱ'?ïûzý¢,»?IÚl†G…?B¶âô?IÚl†G…?í—Ðwfl?À<¿ÝêÆ!?³A|DÀ"?À<¿ÝêÆ!?îøªf'&?šgkâ
Ól? uYšçQ§?šgkâ
Ól?ïðË
;(†?Q°£öèÄ?^iëDöÃÛ?Q°£öèÄAGN3FGL J0747.4+0904@jb`RP/@0ˆçÖyõÀ:d%‹ªÃŽÀ;àК·§?âˆéߓ_)@Hî=à¶9@‡Â?ÖØ¿ÛB¦¿X+K¿Ó $ØÒiš¿àø°ªF(ó¿ãðsÚ AGNbll@ï×XâePowerLawRX J0747.3+0905?ïþŠh½óZ?#)"Â)?'Yv—é?#)"Â)?ïj'ÛN»?£3à"a?'­Ä'~?£3à"a?ïÒÚWú½Ì?p¼¾¹Åþ?v'Ô¶?p¼¾¹Åþ?î'-HQlH?+…B9€?¦Ý+|¡	|?+…B9€?ïöTH_Gí?W=)jØG?SWo§$–?W=)jØG?é㏽³æ]?Æ=ô;j~?ÈqÁ	0f‹?Æ=ô;j~?ïz€›3î?Š–j»	ÖÃ?¯ì¥ì>?Š–j»	ÖÃ?å#&é¬_"?³^Þ7ÒV?Õ¹²,§A½?³^Þ7ÒVAGN3FGL J0748.0-1639@mF÷_²íþ@ÎÙãÀ9/Ã¹þ"À;CÖS^Kæ?õ–qÆì¹@ۖÛúT@Ö[ 9ÆË¿â
^¿èGCˆb\¿ì˸0F¨¿æ@ºr'(AGNbcu@¦{J#:PowerLawTXS 0745-165?ïÄ&¬Ma™?†;U…o?}ì©Çq;ª?†;U…o?èÎítžI?ƕåÅl0U?ÏìÄJ-†Ý?ƕåÅl0U?ï*ýŒˆ9?"+—VŸÿ!?š¼€UN0Ó?"+—VŸÿ!?é2uÚ?¡³×#¡?Éû7¦+ð–?¡³×#¡?휪+s\?µÅ5¼'ø'?³®¥A?µÅ5¼'ø'?É÷WºÑù?Ȝ˜K)¸Ð?鹂*K'?Ȝ˜K)¸Ð?ë¯çŒŸ=Ñ?®Ä»iV?Á@a̓¼?®Ä»iV?Ò¥Cáp?¹n.Ùµ¨?æ­ÞGú?¹n.Ùµ¨MIXED3FGL J0748.3+2401@h'FŸ¸@6­?i¢[À9ÀÜ0À;³Ô&]aÛ¿ð ~ðËډ@[µàÏ8@@`k&¿àñðj¿ä,fꉏû¿áéñd '¿ÕÙ°"AGNfsrq@›Pàù	kºPowerLawS3 0745+24?ïå¼Á֓d?¬âv° A?jC=ýqœY?¬âv° A?ïÚ)ñYã»?…c‹þ?rëR^6Œ?…c‹þ?ïñ¼xõ<á?j‰'ávq?\‡+ƒ½Â?j‰'ávq?ïÿúžc¥8>ºXÀgœÃ>ņƲQ§¶>ºXÀgœÃ?ïÿã"@lµ>ëS®Éœ>ìl›U,Pá>ëS®Éœ?ï9ú?Õ5°?­ð—ÑD5?˜À¸Èæ?­ð—ÑD5?ïë/ʄ._?uvŽd¢»?dÐ5VµÙ•?uvŽd¢»?ïÿФêýÝ>õ^*/E
Î>÷­s¬ñÛb>õ^*/E
ÎAGN3FGL J0748.5+7910@`ß2_c<æ@=GÐ@ÔÀ:›OC427À<)LqMJ?ñj®òÇ2Y@£àÒ¾(o@¿ï©H8?Ñõ%†wRó¿ãæZû#L`¿ç«Gþ‹$¦¿ïÿ¼rÙÞ¦AGNbcu@$tSPowerLawJVAS J0750+7909?é±+HOœm?Ћf5,÷?É;RÞÁŽM?Ћf5,÷?ío¹:7£?²l{þN9?´'6/Î
?²l{þN9?êîLê"—?©ú»·?‹ ?ÄFÌW±í£?©ú»·?‹ ?ê­å"Ãê?ž·Ë´3;?ÅHi°ó¨Y?ž·Ë´3;?äâm+³™?ÓÇéí³»ó?Ö;%¨ä˜Ï?ÓÇéí³»ó?ãÄÀˆ_¤D?ËŸïôð?Øv~ï@·x?ËŸïôð?àò¬&ÜZ+?¿B%¿WC?Þ§²GKª?¿B%¿WC?ت"s'B?±žgœî¨?ãªîÆq¾ß?±žgœî¨MIXED3FGL J0748.8+4929@e$¯ÿ6¬d@=XlÿݛQÀ:3½äÒ}À;âÅû!?ևæ³þŸ®@
­ÍŸZ£»@¶jyÍv¿ÞíG€ù¿ã©;ˆAWŽ¿å¦ÐWN¿îÑzÎþ*hAGNbcu@'AØbMÓPowerLawNVSS J074837+493040?î™d	aJ?µc§p·?¦i¿h3¾?µc§p·?¢I…I?ø™´e…'?Š•~̹­?ø™´e…'?íÂ\_/?œ"Œ…ú?±ìN¹A?œ"Œ…ú?î1Ÿ8¦ ?‰hóß`MH?¬îå9ü?‰hóß`MH?éÊèÒÍþâ?ÃBmÉî1]?ÈÔ\´Èw?ÃBmÉî1]?êiAŒ‰³?Äó+NëÔ?ÆZùÍÙ3°?Äó+NëÔ?ê«$,@`ÿ?°ãU°Zß?ÅSoNþ|?°ãU°Zß?àTÖPì?·áR²•Ä?ßWàS^Ä(?·áR²•ÄAGN3FGL J0749.4+1059@j/
€CR@1˘<eâÀ:¬ÿiÀ;¿­Aí
?Ôpw%?C@™#îq¸)@ŸÈ_ÂX¿ç&J;¯Ðà¿Ý•tè—A¿ãVòì'Zõ¿áKâù×>AGNbcu@™./hیPowerLawTXS 0746+110?ïÿ‰™Wœ?oxRd­?
™¹¶'VN?oxRd­?ïÇw¬ùŒ?Œ÷Ë|`eÖ?|D)•±O?Œ÷Ë|`eÖ?ïìžé‡ ?gߟ	'Z?caA÷ |?gߟ	'Z?ïèFïcá¸?H(nD~?g¹³{Ÿã?H(nD~?ïÿ µ4Þ7?¬™ób?éa{´†?¬™ób?î¯O{`?³(ŠÛD?¥äގ?³(ŠÛD?ïÜ,ÌÅH¨?yˆK¡¯Ê?q陜«À5?yˆK¡¯Ê?ï*F¹ç†¦?†ÃHÈ#x?š·(½çÁ@?†ÃHÈ#xAGN3FGL J0750.6+1232@jì O*à@2»`c'À9c+Hƒ'À;pClfZ¨?ë
ªj³c@VF,	HS@J:Ÿäƒ¿ÛTÌÍ+J¿éX¿Ž˜+'¿âßã鰝¿è Ü/&šZAGNfsrq@‡·KƧðPowerLawOI 280?ïþâ"Ö$K? î/D¹˜?!×±×Ñ×.? î/D¹˜?ïÂu4×Åq?Ž"d܅?~Åeœ\W?Ž"d܅?ïȂç6Á™?yu_zÔO€?{¾Œ'ÛÃ/?yu_zÔO€?ï¸Èyè	¥?YE§Æ*`Å?Íá…ý–ª?YE§Æ*`Å?ïþ´WNà?$VhE,B{?'¸eP€?$VhE,B{?î™|Îv?´¸‹^XÕù?¦o0‹Sª?´¸‹^XÕù?ïRYðØ?'HiUxX?•´ÝET˜À?'HiUxX?5z!?ŒM¼û§?¤vü°œæ?ŒM¼û§AGN3FGL J0751.2+1806@iX;o@5ÏÀ¢À9Ò»úÀ;¨•Š@`B@†äÇ@ïßq<X?ûxt=i—ô¿Ú"DPo¿ÓˏNÖÁ‡¿ã^;÷š¿ï!Õ2!oPSRPSR@'Ši­BÄPLExpCutoffPSR J0751+1807?cŸcv‰¬Œ?i3¯*Y?ïì`œ´{?i3¯*Y?°cöM
t¿?¾"Ð(™H³?íó6BԈ?¾"Ð(™H³?»õÓè[/?¤ù°dõµ?ìŸE'ôš?¤ù°dõµ?®Zkœ¶M'?<'üÝÜv?îYEý¡g?<'üÝÜv?o°Upo@?oàÕ=?þ?ïàOª¦öé?oàÕ=?þ? "v2Èep?²Ò	ñ?îý؜Óy©?²Ò	ñ?¥p,uÅM(?™¹
ÃÇq?î¨ý8¿(
?™¹
ÃÇq?}¢zWKÏ?e«;û×C?ïÄÄ»0m0?e«;û×CPSR3FGL J0753.1+5353@d†A¿½ð'@>…Á?ÐÐhÀ9?ª¹|ðÀ;¨"?…J¿ºÆ^;Ó|@ ®÷#ã@ØúÀP»¿Ñ•º'L¿ãþ-Äx.T¿á5(²7Œ¿ß_~þ°AGNbll@˜¶â'@·€PowerLaw4C +54.15?ïþÖ^4Øi?vûzìã.?"š矘ô?vûzìã.?ïÞ'±°øÂ?{;
;?pì'¿$?{;
;?ïÛX"Œ¨V?v¿ü.5.Í?rS½Ú¨ú?v¿ü.5.Í?ïø՘±?4¹"/Üø*?L©Ÿ&¶èk?4¹"/Üø*?ïþ»‰Z²?!;‰'ôR?$O%j½?!;‰'ôR?ï8x^»«?©òÄAÁ¶?˜ðþmIR±?©òÄAÁ¶?ïÇΞ'®œ?ƒZŽ€¨³?|°§Z}÷?ƒZŽ€¨³?ï·2!Ìi·?tÃgÛ©…?'3wƒž _?tÃgÛ©…AGN3FGL J0754.4-1148@lÙ)¿*å@ y–ÿáL6À8¾2lcÖiÀ;CÉv7]?êÅÐsYN@—M·B÷Ì@á©`6 £¿Ø@)vý¿ãsQŒË¼¿ßMJ!G‰"¿âª¦žS¬iAGNbll@–(g»/ìWPowerLawTXS 0752-116?︯…$}Ê?•6´þíì?ÔÅNéq?•6´þíì?î)=҄­à?ªK;0»[L?­l"ÕýSü?ªK;0»[L?ïaí†^\	?ŒÈ4a±uÙ?"ÂO+xÝ?ŒÈ4a±uÙ?ìÒHïTj?Á¯Î"l?¹m»€óP1?Á¯Î"l?ïPì›c.?"âÖ-Üx?•âl'æ¬N?"âÖ-Üx?àÿzlá2?υñlÐt?ÞÅ&=›?υñlÐt?íƒÏ8?•?¤ÝCeK?³á†=•c‰?¤ÝCeK?ßÑClÄ×é?±ÜGÀ¾4?à^I"?±ÜGÀ¾4MIXED3FGL J0754.8+4824@eQ4 -œñ@>(l <K
À9š0˜N@À;ž"Ž½ž?À¬ÔOß!Ÿ@!eÁzß@$=ÿêÜW¿àêø2†K¿âÏØ°ZÑ2¿âTSK×nç¿ã»´0É¡tAGNbll@"Q4‡ü¹$PowerLawGB1 0751+485?ïý;8 "?1‰ççkT?6&=ÊÏC?1‰ççkT?ïӍèzA)?ƒÿގívl?v9®AÃÛ?ƒÿގívl?ïØ¡$äw?v³í<·Ëô?s¯mŽt\©?v³í<·Ëô?ïÅmÁé2Î?bCÍXd¥Y?}I•å?bCÍXd¥Y?ïô£íÊ7?V*Žlgxß?Vz¸4é±?V*Žlgxß?îÿs<&§?¥ùU…²JÚ? Ì<»?¥ùU…²JÚ?ïa\ÔlSe?'õJ÷xú?"Ôet-aS?'õJ÷xú?íTDtgõ¡?¢¸ƒ–WWÆ?µ]Ü].Ft?¢¸ƒ–WWÆAGN3FGL J0756.3-6433@qTR_ét£À1Â\ÀË6ËÀ9ޟð˯–À;³x«ˆ¤¿ÞtÁ' @atÇ},¦@¼T@(4¿ä"ôµ¸Î¿åM7È2"+¿ãW'Ñ_Ú¿Ù+Ҋ뚲AGNbcu@™r#S&PowerLawSUMSS J075625-643031?ïþn¹'Sh?-ˆÆÂ¥¯Z?)e7¯ÛÀ?-ˆÆÂ¥¯Z?ïÂÌm×Hý?þë
®v?~™Éúi¤?þë
®v?ïé@i z?cú‡I¥°g?f¿èfDþC?cú‡I¥°g?ïüy+v6¤?)Þr…´z¶?<6¥—âµ?)Þr…´z¶?ïüà–-Su?8Qvr¡Î	?8ûN¢–á?8Qvr¡Î	?î¬@™^qŒ?µ±7†Y>î?¥;öndj@?µ±7†Y>î?ïÕ¾`Mr¥?xi,b‹E?u Ïû¢ÅŠ?xi,b‹E?R¢\?rÙëþõ¹?}6®q{Æ?rÙëþõ¹AGN3FGL J0757.0+0956@jiʞõ#-@39 4¾NÀ8"ÕϪ͟À;W4H)?ëÇ:
V´Ü@"Ë'Rz@trŸYÌû¿ãàN#Ïh¿ã£dÃüÆ¿ãq
â秿ã´^zù_AAGNbll@ø»µsëPowerLawPKS 0754+100?ïÿœ]†>þýŒ¥C"9?þÏÐó>þýŒ¥C"9?ïÇ~˜¨?…þ]Ô̔{?|@³ã=šÊ?…þ]Ô̔{?ïæGËNP#?gΑfí?i¸4Ό•"?gΑfí?ï§4LìJt?aIý®MÒ?†2ìË̚î?aIý®MÒ?ïÿxhœv™?ðévN?òóû	Éú?ðévN?îe÷>¡Œ"?·qúf›j?© ŒzëÇ?·qúf›j?ïÏB×Ú¶´?€S¥QZQ	?x^""rÙÚ?€S¥QZQ	?î[ù·?•¼óÀñ|?®Þ_¬¯'?•¼óÀñ|AGN3FGL J0758.1+1130@j=ÒàãG@3õ[_¢'À:_Y²"ý[À;ÒNér?çMÒ%U@G®¡hšô@QFt›?à‹!Ω=H¿çM>Dð[¿Ò@bÒn]'¿ëJ¥mQ+AGNfsrq@œ©·KƧðPowerLawTXS 0755+117?ïøØ¢Ô	?Iø­*²1Á?LŸÐsf¸Û?Iø­*²1Á?ïZ7{cÅð?œ9ïÀ
ÕC?"¹šfz?œ9ïÀ
ÕC?ï.(˜Hb?ìðð?š:í&²?ìðð?îZ4	C?ŠmZ.FOË?ª^¼Ü&Í?ŠmZ.FOË?ïïñ:H?bzRXžÆå?`ņ'žª?bzRXžÆå?ë`Ö
àŠ¼?Ás¹±Î*?Â|§È}Õ?Ás¹±Î*?îË"ͬò?™¢(!Ø?£Nö²IIè?™¢(!Ø?è綊7žI?³¥ó£ô?Ìa%×!†Û?³¥ó£ôAGN3FGL J0758.7+3747@fÕø -à@<àu¿Ÿ½ À:—±æ—y.À;û>ß8à¿ÓX¹mR‰@sŽíï@>¥ 5"?ç‡ShTJ¿á'[ËF©¡¿ärÜDäá¿âÅz·pAGNrdg@˜n¨	ԕPowerLawNGC 2484?ïþ͈çù,?%
;úñˆD?#'nRÉɉ?%
;úñˆD?ïÛ`ßqr½?-4ÒSÏ'?rOP5ª?-4ÒSÏ'?ïÈ¥#e‹?uŠQc³ Y?{ö-‡ºVx?uŠQc³ Y?ïøÑ貏?6'¾€Cà<?L» MÑi?6'¾€Cà<?ïý'›¿þL?5¹¼öZ?3ë#æ	?5¹¼öZ?ïªKÔ¥ð?­sIq	ÃÓ?œŠ¶…kAö?­sIq	ÃÓ?ª›þ?ˆÓ¡Û»×?ŒUUãå?ˆÓ¡Û»×?ï©·ûþ?|½•¼³+¾?…'8½ã ?|½•¼³+¾AGN3FGL J0758.9+2705@hI#ßm¹A@9òσ³~À9ù"'Ñÿ<À;ÓËwb7-?é]:êGî@†lQöÃ@ —пæýGÜb–ù¿Ùæ×Ê°¿Ü7£8Š¿ê驀'¾ÇAGNbll@—»»J#9ÁPowerLawSDSS J075846.99+270515.5?ïyv¾Î1|?[ŠA]«?Ñ($'‰?[ŠA]«?ìf,|,BË?¶s‹¼("?¼Îœé¤?¶s‹¼("?íï–Ú]À6?¢M±Ñ-û?°ƒI.ÉÌO?¢M±Ñ-û?é'Ö7•Ô¤? nà;ø%W?ɸ§!¨­o? nà;ø%W?íD´æã4©?´?ïì?µÚXÉÂA´?´?ïì?Úwße&d?Ít‡ï֛?âÄvMlÎ?Ít‡ï֛?ês!GçT?°§D€w.—?Æ3zã˜b¯?°§D€w.—?ќá-Ôò?³E¦°Ðº?ç1@i‡?³E¦°ÐºMIXED3FGL J0800.9+4401@eø6ŸÏ=À@>‰M߆ã´À9ë̗ó§,À;åáMQ?áÎn"w	¼@
dSÉ&@X?Ý»¿àJÄë	¬Z¿ãžK'gµ¶¿ã•ßû¨­^¿ëǵn6itAGNbll@‹Ž³œ¾àPowerLawB3 0757+441?ïæ,À[
?g¥Ì¬NL?iÓ?à:Û?g¥Ì¬NL?ï¬k3æȈ?"[òF'aE?"å3N?"[òF'aE?ïCp¡ÂvÌ?‹"–)?—'뉼}?‹"–)?î«í¤ç33?~$"À(ځ?¥A%±ŒÌÏ?~$"À(ځ?ïvD¼áB?'ÓŘ?'7h£×¿?'ÓŘ?ìxŠGìþ›?½"\¥¿º?¼;­À˜$?½"\¥¿º?í(<O´X?¥g‹fB?¶¾†žv??¥g‹fB?åÆ¿8~ez?°$pú?Ôr5?°$púAGN3FGL J0802.0+1005@jw6â—@46'ßk5À:`2g[XìÀ;Ô:0}vM?ÓÈì²44@Œsk\š@*‡?Ïε?äø‡ç2¿×õ)¹Hß¿écí°r#3¿Öåæ<2AGNbll@ŸhÛ=ÈKPowerLawNVSS J080204+100639?ïûCìz"l?MþŒƒ‡IH?BðM:‡K?MþŒƒ‡IH?ïÌhåá_›?"fÀL›?yˍŸ˜?"fÀL›?ºÀl?ƒÂ6/ŒÁŒ?~T¿€ü?ƒÂ6/ŒÁŒ?ïÌ4µÙ,?bx+™óœ?yå¥&»¹©?bx+™óœ?ïá8^b®B?tëø®s?nÇ¡}µUÁ?tëø®s?îšîHÑÎ?±é`ã¤ès?¦Qp[Î+?±é`ã¤ès?î7v¢ž¦?£mh¥e<¶?¬è˜iʝ?£mh¥e<¶?íaÜŸl?©dQ]F«V?´ñ™¹ª$?©dQ]F«VAGN3FGL J0803.3-0339@lƒ@'À‡@,[	 :2+À98'ódKÀ;kՙ$(Ô?ÓNЦ(ѹ@÷êï!¶?ÿðÁ¡J'ö¿à<ÐÀ¼¿á6‹ÐêO¿Úx¯IÑ}¿ã&oI¨¯PAGNbcu@³y#¢œxPowerLawTXS 0800-034?ïþï	kAJ?AyEå?!k&èó?AyEå?ïÅŠÌLI?ŠnŸûƒˆ?}v:ƒ,os?ŠnŸûƒˆ?ïíùoíù˜?dÀëHµ?bÔ-p$?dÀëHµ?ïãÂÄÇV?K¿tÝV‡?lâ=Yu9Ú?K¿tÝV‡?ïþL3Õµ?'HµŸ3_r?+<Ñìk(?'HµŸ3_r?<æKŠ?³õ%5Jã?¥—l5
ãY?³õ%5Jã?ïÝh¤6ß?w"·ð†¸.?qK­ßÁ?w"·ð†¸.?ï@A¤>a?'=|‹4‡·?—÷Ë~3Ó?'=|‹4‡·AGN3FGL J0804.0-3629@o¡œýç!À-ŸöUÀ9JⴕžÀ;êßÝJÉ?ôUi"í];@>Q%âg¿?ýAŽàØóL¿ãw»3®i?ïõÝà£÷Ê¿Í@X¤u¯s¿âŠ­)楳AGNbcu@´õ×æšÔPowerLawNVSS J080405-362919?î©&é4Î?§^òėv?¥m'hr°!?§^òėv?éƒaQ‡9Î?Ǒ/ª	 ?Éòz¹ãÇ?Ǒ/ª	 ?î)|'eA?žÁËÛÃÝ%?­h=†<Rh?žÁËÛÃÝ%?ëÐÖÚö8ß?¡ÄÅÐÛÚo?À¼¤"''?¡ÄÅÐÛÚo?ìîóàŠ?·"
&¤£?¸ˆgÿ(û³?·"
&¤£?Ý{u^HW)?ј{vîÉÍ?áBEPÛÔk?ј{vîÉÍ?엾M¶ŸÂ?©³Ø~¨À?»B
'Kí?©³Ø~¨À?æø't7'?º|Bõⴄ?ÒÝó'³?º|BõⴄMIXED3FGL J0804.4+0418@k/òÿÑÜ×@2/ Z8[À:9Íp`»,À;Î ž9%¿²ÿÖÈû¼6@bÎ
{@‡¾?Á6¿ám, 
樿ìSò²ÿ¿âu-yÆH¿ØŽV,\AGNbcu@ƒÿóbb˧PowerLawMG1 J080357+0420?ïÿÑ¿ÙQô>ô5qKýèè>÷ 4'Å'­>ô5qKýèè?ïÑþkðõ?ƒœ·®¾?wÉéÂu·?ƒœ·®¾?ïޓì†{…?yìªl^zÅ?p¶	ž…­Ò?yìªl^zÅ?ïü#þsA?$õ#Žj{?>à§ìþ•?$õ#Žj{?ïÿÓ,ëÎù>ùå!{?>öi‹ó€›_>ùå!{??îöÅe
¬è?«pvÐ4îò? "©®yJ{?«pvÐ4îò?ïÒg¨±`?y´Vª¢Óš?vÌ+Îû$H?y´Vª¢Óš?ïØénKÀ¦?guÄߌÒÀ?s‹HݏHÐ?guÄߌÒÀAGN3FGL J0805.0-0622@lj	 'RT@*iݾŒ˜)À9Ð%E3æ·À;sŠ÷?g¿¹QQŜ6?@(©€—j?þQìa<°à¿î~»Þ?Š¤›£M¿â½Y4N¼&¿Ÿ+ÍÊ^ï‹AGNbcu@±™c•%PowerLaw1RXS J080458.3-062432?ïÿidü?"cˆ×OÁ?òÕÙÐâ?"cˆ×OÁ?ïξœø
?‰<¨/bÁ?xõ £¼?‰<¨/bÁ?ïåÔÀ·Õ?e(^I0¨n?j+?]ˆÓ@?e(^I0¨n?ïþ%Ã;²?¥Áu¥6•?-£Íb¾x?¥Áu¥6•?ïýõ}Åþ?1ø8,Œö?7èT¼<«0?1ø8,Œö?îõ0ºn6¦?°˜-ãÜì|? ¬ôZÔc¤?°˜-ãÜì|?ïÍ7žQå%?}/ŽñD…Q?yd0Ö]}?}/ŽñD…Q?ïìth:Y¡?ZòI£þë?c‹—í×?ZòI£þëAGN3FGL J0805.2-0112@kÖ3?Èlì@/—(_ššKÀ9"ÛVÓKÀ;¸Y_æÌ?àBñ¿þæ®@?ìsS4@·ô`d™³¿Ùv'D"E¿è4îV,¿áÄìÿUK¿è²+¸YgAGNfsrq@‹|\'ÆPowerLawPKS B0802-010?ïÿ¡®;N?"Þ†d¯?"iÁ¤ÚÅ?"Þ†d¯?ïÌN"Us?‰6ÿLz!Ç?yØîߕS?‰6ÿLz!Ç?ïÖ´gÙ¶ž?x°š q~?t¥Ìs…?x°š q~?ïì1ÿ¬s?Bs ¼ëÔØ?cÎCÏÿ?Bs ¼ëÔØ?ïÿ†%§'?ýßrôn{?v‰œeï¦?ýßrôn{?îÁméÆ
n?¶ü.·&?£é!gêÜ?¶ü.·&?ï­&zyT?ƒ¯q½?"¶ahŠ3ô?ƒ¯q½?ï™ólÚÚé?uí¼sõ®`?‰ƒ$ÅÙ©Ú?uí¼sõ®`AGN3FGL J0805.4+7534@a\j~ùÛ#@>ʙ÷LÀ8Û+6¯ÆÀ;s}°/U¿ú'Cß}Ôl@;ôvH?þ®íÿ!ˆ¼¿ÙÁ‹EmóN¿ß©Æónø¿ÞMdâ­µ¿ÑkFÖºG AGNbll@ŸˆüÚQPowerLawRX J0805.4+7534?ïÿÀߟb?ˆÅKˆ~>ÿoS
o?ˆÅKˆ~?ïۃeÍu?†:D J¶?r>qÆ:
L?†:D J¶?ïÞ{֐?zÏSuU?pÂ¥e?zÏSuU?ïÿý? Ò>´ gvJá>¶çØzÒ÷>´ gvJá?ïÿs¤×)6?ZW6É­}?‹dIñ¿?ZW6É­}?ï=­–W?¨®ÊNH?˜^
]5?¨®ÊNH?ïìõ0,?rl8õ)aG?cø
²ÈT?rl8õ)aG?ïÿ׫øì»>÷ól…#>ô*åk™»>÷ól…#AGN3FGL J0805.4+6144@caA?ÐÐh@@.é€aº/À9öåvÀ;ãe§ú…m?ôIYÑÇÞ@_!CœŒé@üº€™îS¿ãã•Vœwx¿ëo¼™Ï¿ëÔ5™6j¿ïý2È1æAGNfsrq@u*°ž˜ÜÛPowerLawTXS 0800+618?ïñ#Zð‰?rtN¬A"2?]¹û¤ÔÀ?rtN¬A"2?ï×lGyø?€MF<ùÓ:?tIðº–Ø?€MF<ùÓ:?îõÆÉ'¦¸?"eGXÛÄ? £"jø"?"eGXÛÄ?ﺩXBP ?aB!"»?U©í=è?aB!"»?ïù×5A¼t?Jld28VÛ?H£*k7éÝ?Jld28VÛ?îìˆd‰ö?®÷U7"4?¡7~é·`¡?®÷U7"4?¤Gë?žO¨½V•Á?¤T®4ߚU?žO¨½V•Á?ïE
êé?æ$‡Ø×?Ÿ×^K9å)?æ$‡Ø×AGN3FGL J0806.6+5933@c³û_ïJ@@J˜?ýFÀ:c/Çmè;À;ïÅôkwGÀ`
+Òí@(õgJ¼è?þ€W([¿ïòÌÒÅÎñ?ïK™™C³^¿ëĎ*XKÏ?Ôb­WD=$AGNbll@®7jdÂø8PowerLawSBS 0802+596?ïû4B
&ë?PÕÛBÌ"l?C.øY:˜Ã?PÕÛBÌ"l?ïßsf<?ƒQ%¯å|ñ?pFtç/:?ƒQ%¯å|ñ?ï‰&¾Êoi?"ºˆ¼!å?¶PCQÂ?"ºˆ¼!å?ïÿÿÀ¦4>"°S"Ún>Æ+"F>"°S"Ún?ïãY&j€…?p™Œ 9ÒN?l¦Ù¬ÜÒá?p™Œ 9ÒN?ïs^Š¶
)?—	ÉϹ³?'".¢_"ì?—	ÉϹ³?îÒN""Æ?šâ=¦Ž?¢Û½[Ì¢?šâ=¦Ž?ïÿíÑTEý>õ€á(¿ÝS>â.;ºw*>õ€á(¿ÝSAGN3FGL J0807.1-0541@l_?p]@,Ï¡"cÀ8Ât=¿~0À;BñTk'?ðM¥&À‰@2^?Pwè@‹°ÀQ¿:?ɒ˜Y¿àŠÚ‹É™´¿àÙ"v€›¿æB£•4ÉÐAGNbll@šio·éùPowerLawPKS 0804-05?ïÿ[ÈÜ/õ?ëv7åKÎ?†åü'jª?ëv7åKÎ?ïvb	µ`u?Ÿ(—{"?'3¾Ð3)e?Ÿ(—{"?ï¿V>rxæ?{Ï;@5¹?€*p_š4–?{Ï;@5¹?îàqø?í+?v¼šÉô?¡øàwµªX?v¼šÉô?ïþµ·©Ç\?%7wmD~9?$¤Ýð˂?%7wmD~9?ìÜ|Ú¾tg?ÂÆIÒÿ8Q?¹*zPI?ÂÆIÒÿ8Q?ïe"îi
?'—9sèOÍ?"MbBòS?'—9sèOÍ?ëeǬG?¡Z^µõ|?ÂhãñNå?¡Z^µõ|AGN3FGL J0807.1+7744@a
¿p@>tþÀdß~À:*‡{‰äÀ<D™`¿é×s¾àóB@Ë,çêŠx@}/`jÎÖ¿è°—YoÕ¿åô©Ä\ß¿æµ´"xít¿â
¢ûd‡6AGNbcu@Š‡ñ!«KsPowerLawNVSS J080637+774607?ïÿÒªÿ"î?!öÁã>öª{A#µ?!öÁã?ïáòYNP?~tԟöF?nâ
"Ó¸*?~tԟöF?ïΧõ‡?}~Eº¦,ñ?x¬~ßh4º?}~Eº¦,ñ?ïÿšë[á±>ø#MýÉ?	E4Îß¼>ø#MýÉ?ïÿ_È"Õ(?O >)?ôђVþ?O >)?ï3L2* ?«`èBâV?™–y¾,×í?«`èBâV?ïŽ_•Mí?ª*>öi?ŒhžüTÜ?ª*>öi?ïù"ky?DrÑ1ëz?I¯ãóSf?DrÑ1ëzAGN3FGL J0807.9+4946@e'ŒŸ¶M@@9»üÊÀ:$B_öàÀ;ò©1½n?ámyÜK@Q'H—sz@"@ªÀ3¿âœQ:7çÖ¿ãlº4ç	Ü¿ïÿô³à[¿Øùå!ŠòÀAGNfsrq@uÎ!–R½PowerLawOJ 508?ïþß¾|?'`íumôR?"«j˜?'`íumôR?ïд:&8ñ?'Ú9¥Ïï?w¥âÔ&W‹?'Ú9¥Ïï?ï²²{#"?}T=;Ä*(?ƒSaHÍ{?}T=;Ä*(?ï««þ²3U?nyEøCq?…L"òà?nyEøCq?ïûòè?PÎyšª¡Ž?Cϓ;J7?PÎyšª¡Ž?îX¹ÚN7?±@®† ?ªtbW¬òä?±@®† ?ï«'=Õy?"vH	BÄ­?ÊÑf÷?"vH	BÄ­?ê™:¯\;?¹OBܔ-.?śBû?¹OBܔ-.AGN3FGL J0808.2-0751@l¡qÿ÷œ"@*Vì¡~jiÀ7/¬ÎÞÀ:¨Æ¨Æ]G?üˆ—'ÃÊ@«i«kG?þÕ¨%xŠ€¿Ý7I²~¿áå=î¿âuì¶wò¿æX|v{ºêAGNfsrq@'Jw€4mÆLogParabolaPKS 0805-07?ïùç"x?U"Dgtî"?Hb|˜Ä`?U"Dgtî"?ï·6Cø—?—…£Ãi Ö?'2o8Ñz?—…£Ãi Ö?î-ÛËËÎ~? Fe€gf?­"CGŽ›? Fe€gf?ïÿ¡1,b?-ír,?«Ú.äò?-ír,?ïñ-t5?`«ÖFÿ?]ó¤ÛÂî?`«ÖFÿ?î¸÷M(ý¥?µEÕ«¦^?¤p‹/'ó«?µEÕ«¦^?î®S‡ ?Ÿ
aüð4?¥Î:õš-?Ÿ
aüð4?ïÿoÇc+s?"é¸_¾ˆ?ü+ëv?"é¸_¾ˆAGN3FGL J0809.5+4045@fzX`f@?ŠüAÿÀ:-Ÿw),IÀ;Ò½M#Ÿ¿ðÂ^18²#@Ô¾È}1Ú@3
ŸÐÀL¿åŸ"úÚbs¿éz§ä5E¿àF…8ʲý¿ïþ÷b³º"AGNfsrq@'C¾
í(PowerLawS4 0805+41?ïÿ!™óË?ú‹r̓?ÜÐX·©š?ú‹r̓?ïی÷'qè?"
,jƒå?r9"€4È$?"
,jƒå?ïÇÉÙ¹€{?g£E&ì!(?|vŽ?g£E&ì!(?ïÿ}'If?
ZRdü
?0M՜™!?
ZRdü
?ïÿ²ºýÂc?yä'âìR?QBXÌÒÂ?yä'âìR?ïÇʍ
?³¶úFZ?œ§°Še?³¶úFZ?ïÚiÛo'?u šHýà?rË^»šö?u šHýà?ïòÒô•Ní?TÇÕ§B ?ZZ£çņ?TÇÕ§B AGN3FGL J0809.5+5342@d' 6m@@wÂ`b@gÀ9ì¿G©ýÀ;èÊõ\8?ÀµÿÅêÓ@ð›äøg°@A)Þ팿ßC߉¤X¿å÷Ù<5ª ¿èßÓr-nù¿Û¥Æ]ÇÜMAGNfsrq@‹gŽ¾ß¤@PowerLaw87GB 080551.6+535010?ïÿÎ9^py>üÀmÛQ>øãCCa—>üÀmÛQ?ïرå"?…ÅJrKR?sþ§Jf#?…ÅJrKR?ïÙç2«N?f#ÁUÁAÅ?s1wLß?f#ÁUÁAÅ?ïú?HŒ®?/d…y3?GÞ}ÀO7?/d…y3?ïÿˆ›fðœ?K\.Ý4#?
Ù#½U é?K\.Ý4#?ï'¯Õ×H¸?«5ïÈqÀ¯?›
>7±
?«5ïÈqÀ¯?ïQ	xà͜?"PõLv?•ÞÐàv°ˆ?"PõLv?u‰‹üÅ?s«'î~öÈ?€ššñ
¬?s«'î~öÈAGN3FGL J0809.6+3456@gNà @À@>Y³¿µÀ: ¿ž(uÀ;›]np $?˜³âèdzJ@Ñ$—'?ú´WÀ±5˜¿Á½~r™?ï ú!Ô
àäíç
¿á©²;&ÉAGNbll@³ÅOß;PowerLawB2 0806+35?ïþœL@9E?'ÌA žO?&;?Þº–?'ÌA žO?ïÜjO»:d?výEÃ]'B?qÊØ4@Å´?výEÃ]'B?ï»Ó͔jR?ƒT%©´!?Œw‹?ƒT%©´!?ïäÊòy|?TL6¢›ü@?k5
Ë?TL6¢›ü@?ïú³°;E?G×pçäS?E1@-Ž(¸?G×pçäS?ï]Þé–?°nÞ¸þ%ð?Ÿ"D)¬u	?°nÞ¸þ%ð?ï½ßê5éF?ƒãâN?€ˆ}"nq?ƒãâN?ï\'h´»?‰K>òÍö?"m²ð^ •?‰K>òÍöAGN3FGL J0809.8+5218@dÈ,ÿ§ël@@tw_²íþÀ7¦&áìÂÀ:É×5Ü[?ÀåRÓµ@¼ãÊ?SÓ?þ‡ ›+¿á"P$c?H¿Û@°ÛeÒÿ¿ÛÊ¢Ú¤Àƒ¿Ø	ŸÚÌAGNbll@™€FYJôñPowerLaw1ES 0806+524?ïÿ¹qƒÙq>ø‰w>Df?£¬%YAb>ø‰w>Df?ïÜjÄÄë'?'uc…µä?qʝœÚS
?'uc…µä?ï֖˜:ý`?|Rxt8<¯?t´³ÞaÈ9?|Rxt8<¯?ïÿïE™V>ўñ'‰%>àýz™†3>ўñ'‰%?ïÿp›sŽm?¾
±ÊF?ì—,Ì9T?¾
±ÊF?ï^d!Æ+ü?˜±~öQÁÄ?"3{À[H}?˜±~öQÁÄ?ïèK6›XÈ?x|ËÝ¢?g´ÉUˆðl?x|ËÝ¢?ïÿÞ;×hÿ>ïG¥=ҏó>ðâ惸»>ïG¥=ҏóAGN3FGL J0811.2-7529@rtÿ†]}À5n -1'À8H°?)áÀ;hþÇÜ¿¢Pä®qÁ.@t]%ÊêÊ?ÿ* Htä¿ßÌwgjX¿ß¿Ùwˆ«=¿Üб€7•¿ßæ.<îAGNbll@œ÷†s×ÜPowerLawPMN J0810-7530?ïâ hw°?‡~ÙÝ~N?mߗ†ð Æ?‡~ÙÝ~N?ï·WL9‹ß?•¹à‹ñe]?'*,èV=?•¹à‹ñe]?ïoî¿)ºÓ?(ÐpÕ±÷?'(€s–?(ÐpÕ±÷?ïÏ¥œ‡5?d9ò¾Õ?x-OI	x?d9ò¾Õ?ï‰vÃÍ?sý‹ƒÐ?¢zK"À?sý‹ƒÐ?íÛsÁ÷9f?¼É>¢Òþ?±$aïØAT?¼É>¢Òþ?ïUj"r?–z"®å?œ•R¯q¿'?–z"®å?íՎ5s'?¢žÖøÓD?±SŽTÑor?¢žÖøÓDAGN3FGL J0811.3+0146@k–gk*@2Ž³ÀŒLªÀ8NâWxŒÚÀ;6~	ñŠ?æaž39ñÇ@HUñ¤ª@D¿Æ©ó¿Þ‰ÚÈ/|¿ã¬Þâ貿àÚWí¢'¿åÿa"<AGNbll@ûw!Õ<ÞPowerLawOJ 014?ïÿ±KŃá>ûŽ†ÝFQ!?­Ñ>ûŽ†ÝFQ!?ïÏsûœ»?‹"bm·?xqF	ÚJ?‹"bm·?ïí Í*Ñ?Rø3»•Ù ?bß2ýƦU?Rø3»•Ù ?ïó‹:[E¡?;´³­?^}?Xé‹Çæ]h?;´³­?^}?ïÿ~Zu?hóôŠ±÷?4¾®ð´?hóôŠ±÷?îÄFcð?µÇe	Ö¶?£»™Âµüå?µÇe	Ö¶?ïâ8:È–?sßµ¥¿?mÇÅ_áó?sßµ¥¿?ïÓ$š
¥?g]C™ß?vm³ûi?g]C™ßAGN3FGL J0812.0+0237@k¢ ¼8*@3=`³žþÀ:þ?5ŸõÀ;'ÕÝÀ¢"^#Í@€èÏa҃?û"éž¿ž;¿äGzr.h¿ásà¸ù"¿Ôê~DdÅ
¿Ã—
f>AGNbll@·í"Iº^PowerLawPMN J0811+0237?ïÿ4ïS"?͋Mâ¹P?2¼»¡Äˆ?͋Mâ¹P?ïØ,Þ°¨?ƒ›·Ð¥ð?sé'…?ƒ›·Ð¥ð?ïÝzlWÂ	?yïE/ýy3?qBÉì,?w?yïE/ýy3?ïÿÿÿv¡>2'™Š¡¿>7ñu=<U>2'™Š¡¿?ïÿt\µ?EKþȶ?}®´…©?EKþȶ?ïWðÆzs?›ßv¯‹J?•çC˜š?›ßv¯‹J?ïׯÈL?‰Â%E?tx¨[žú;?‰Â%E?ïÿÿâxۉ>{Žrn¶'>mg™ÆN–Ó>{Žrn¶'AGN3FGL J0812.9+5555@d> öð@@ºö€$}ŽÀ:3b-À<¦J'R¿²©É{TLB@Œ¥{úø@ã; 2¿â´®<œq¿ä'§n™e¿ââ~=%X¿× N+S=AGNbll@¢4Çy¦µPowerLawNVSS J081251+555422?ïÿVm'©E?
áGÉÍ*ø?2YeòÄC?
áGÉÍ*ø?ïÜ%?€8Üç3lÊ?qñmg¢Ö£?€8Üç3lÊ?ïáÞ~ðç?mJúCØ?n!ÆóP»?mJúCØ?ïî/Ñ\‡?IöåמÀ7?aðÏïj©;?IöåמÀ7?ïþàŸ°4?Қَ3#?!ÿ•Àš?Қَ3#?î̀.8¢‰?±Ó¡!ôÄ?£7ýu×s?±Ó¡!ôÄ?ïÐGÜôž^?wBÛÆ´‹?wܝ(Å?wBÛÆ´‹?îÈÌZ¿?™	ŒaEìÔ?£ƒ<ç»0?™	ŒaEìÔAGN3FGL J0813.3+6509@bÝß֔Í@@€0`À:Ž'‰ÚßµÀ;Ô¨·CΌ?ϛXŒÍ@
R¢Æ>_@'°?£Y¿ë	G¨'¿Ûw­ÕL¿á:,‡Ù¿èÀ—Ë@ä)AGNbcu@£Ô ě¦PowerLawGB6 J0812+6508?ïøC ¾¦ï?Q†ç†P­h?Nñ}
–?Q†ç†P­h?ïÓ?`Ï3ë?€=0ñ?v`O&úN?€=0ñ?ï´â]¶G-?ƒ©^'r.?'Çh‹ŽüÎ?ƒ©^'r.?ïŒXjœ£\?oR 	½õk?ŒéåQ÷ñ?oR 	½õk?ïç=Ý?qí[×Ñì|?héû6º¢¹?qí[×Ñì|?î0ª»¼?³6†sÓàˆ?¬õTFÒm
?³6†sÓàˆ?ï£GÿYM?—K[Rt±?œ‹—"rU?—K[Rt±?ë-›<9Ÿ¼?®±ñ̂ò[?ÃI"?®±ñ̂ò[AGN3FGL J0814.1-1012@lütÿ†]}@*m{Ÿ³À8ú"mRÀ;L†ŽúÚ&?Åzm]À>c@K9Ž—@'8`Är¿åÚîÄÕmÁ¿ä˜¢dT¤ƒ¿Û+z	ää¿àDžt¨QAGNbll@t­«ŸU›PowerLawNVSS J081411-101208?ïÿ&úsVÂ? 
y©Bé? °Ærh? 
y©Bé?ïʏÃ×Ü?Šn0
b?zó¸Ãþ0?Šn0
b?ïŽÄe?iÍ·|-K?aPn|:[A?iÍ·|-K?ïóÙZòm?<ð!½7Çq?XMI¥¶–~?<ð!½7Çq?ïþn €9\?)4Ä3ù?)ô\mV¾?)4Ä3ù?Ÿ‹˜q?¶™3»æ?¥¶–þFæ?¶™3»æ?ïâhà
¹?|È­Šê©?m— âÙ?|È­Šê©?ﬠlœ‹f?s
X¿xí"?"×äÜLÂ\?s
X¿xí"AGN3FGL J0814.5+2943@h£3v@>€'ÍÀ:y¼>§À;ëtZÏY?㪛u(@
O
–<?ÿ¦à©ùc¿îí(ށ¼>?èŽR€«a¿àÜbSS±z¿å÷/"ÃAGNbll@§/$?åÉPowerLawEXO 0811.2+2949?ïý¥OãË ?@eï eÈ?2Õd2À?@eï eÈ?ïweÂûy?""36Î?']ÁXì?""36Î?ïהáùÚ¢?pS^™4ç?t5pä?pS^™4ç?íø?,nPž?')‹ï«×±?°>žEI?')‹ï«×±?ïî«izº?bæq¤ôF?aTç[kýÿ?bæq¤ôF?ëZý#y#O?Šñs}Ù¨?"rrÅ?Šñs}Ù¨?ɧ?‹mˆòììß?ŽŸM_@ô?‹mˆòììß?ã°±Ð5ü«?¸ôA†J@ó?؞œ_"ª?¸ôA†J@óAGN3FGL J0814.7+6428@böW´@@›aßîèÀ8Žõs}¦À;}ЍK­}ÀٔPXÞ@ú­ê^ƒ@_û¿~…—¿â{fôîC¿æüN^v¿à¯±íè@¿ãNŀ'W³AGNbll@R½<6PowerLawGB6 J0814+6431?ïÿØ´>êQ4þµ>óü®@³Ê>êQ4þµ?ïâ‡
î?zöí\bJ?mxõNgj?zöí\bJ?ïòi;?V8Uú?[-õ'é­?V8Uú?ïÿÿkIhî>'R%¥
>'c؏Ě>'R%¥
?ïÿÈqÀ®ÿ>õj»´Å''>ûÇ%W`\j>õj»´Å''?ï[5ÄÂs?¢ŽÕkä+?"™GwM?¢ŽÕkä+?ïï%|ç?eB›_‡D?`Úb—8é?eB›_‡D?ïÿõf§‡w>ßNK‡iF>Õ2åã€\ã>ßNK‡iFAGN3FGL J0816.4-1311@mYb¯È°@(AŸ˜À8cKB±ÂÀ:ßÄ"ïï?èÝÌ.A[ë@ß²ì¦ÜÎ?üméµí¸?hA¿µY‹¿áÔ'€]Ē¿ËyÓ
D¦¿ÛL'æ>ZPAGNbll@©ª~ùÛ#PowerLawPMN J0816-1311?ïÿ\èŸwe?05K‰Ìà?béw6_?05K‰Ìà?ï±^q?'6'?›1°?ƒ¨|KÛÅ?'6'?›1°?ïÓ±óB"?yYÁÙÓí:?v'u|þ&?yYÁÙÓí:?ï֘x‡?SŽAÿâ?t³ÿÆ|*8?SŽAÿâ?ïþµÚß,?)ŽH̖èg?$¢`܃¨?)ŽH̖èg?îW£6j9?¹¥®eXŸS?ª…Ì›ð##?¹¥®eXŸS?ïÛ¢ÐFvS?{0Ù!¨ö÷?r.—û±R"?{0Ù!¨ö÷?TÜÚ?yº|¾¦‹?ŽÓ¸‡9}?yº|¾¦‹AGN3FGL J0816.5+2049@iMfŸê%@;¦1_ô\^À:™8I©"À;ï"öW
?ÈJ]*lT@
ž‡½N)¯@?è`&0k?¸2Çä–Ô)¿Ûv<lí¿¿Ùì£{^‰è¿éf"6Þ'AGNbll@¢ÜÃ9ÀëîPowerLawSDSS J081649.78+205106.4?ïãXy‹(µ?na¢…œ#Ç?l§†D¼ÃK?na¢…œ#Ç?ïÑçÈóñ¡?}ûp¸Ê˜\?w£"Ó:?}ûp¸Ê˜\?îëö"±…Ê?˜¯Ô+\8?¡@ÖŸqe?˜¯Ô+\8?ï©É"«jŸ?fD¶õʛ?…šÜB?fD¶õʛ?ï|[N"?''1hÂ\?tŸÚ¾a?''1hÂ\?Àø
ò?°q¤¬?¦'³ðPå?°q¤¬?íVÓhiÃ5?ªG€P«Ï?µId½ûÀÚ?ªG€P«Ï?í6k
Ô´?¢Ð‹ÖÞ*?¶O\¥ñŒb?¢Ð‹ÖÞ*AGN3FGL J0816.7-2421@nŠÀ€ù£@ïÝëÙÀ9HÏmýÀ;ohی¿­r†fSJ@Pkþ*é@thŸÑ—¿àf¾ ȳŸ¿ç¾o+ÜÒ©¿è^Ξw銿ÛîÂôdtAGNbcu@‡cF?PowerLawPMN J0816-2421?ïÿhûìõâ?¶¢lKN?àŠ«RqB?¶¢lKN?ï¿X±iD?ˆ¼p'JÒÊ?€)üÎÖ;?ˆ¼p'JÒÊ?ïÊS¢®/?vM)£,?zóÖÌ0?vM)£,?ïü"u#~Æ?$^>áa?;dTï¯`?$^>áa?ïýÌüó[,?8ñÏÝ/*\?1˜c#XŒ?8ñÏÝ/*\?î7?C%³]?¹¾'H'È,?¬ŒͤÊ5?¹¾'H'È,?ï9íc½Œ
?•/Ûý?˜ÂSuèÈ?•/Ûý?ïÚÂkpÒ?gMU2^dv?ržÊmè^û?gMU2^dvAGN3FGL J0816.7+5739@cû;@³Nw@@øÍ?¹SsÀ9¦Üx;{À;¡iÀŽ¿çð+‰y@mJ
jKÎ@ç@ó¿ãýæzÕé¿àǵ…Õ¹Ó¿ÙÖ͂»lä¿çj…QãøbAGNbll@•KFö"FtPowerLawSBS 0812+578?ïÿ—²¹¦)?Û`t?
[¿v×9?Û`t?ïߎPmß?¿xØ%?pw8Òùœm?¿xØ%?ïòeaÒ?P6àð_{†?[5Õ¾ÿªÔ?P6àð_{†?ïþ?Ž5bb?‡.Ã]?, ‰œFv?‡.Ã]?ïþ ÒHÝ?'>v©ËÙ?%òÚX–ß>?'>v©ËÙ?ï=ÒV' _?­Û?2ª?˜Eµ8Rú?­Û?2ª?ïèÅÖA?wK%ó¤?gÿ:!Ò¬?wK%ó¤?ïì|V¬xÞ?^ž––Ífò?cƒ©lDQ·?^ž––ÍfòAGN3FGL J0817.8-0935@lúš?Ffí@,¢9 4¾NÀ8ß¾®&˜À;G²3ÄR«?笃›‰ù@ŒO¥¯§x@YIàsÈ¥?§t¹f#Ý¿Þ7Áá
,¿á3צx,ë¿àï›þ< 3AGNbll@œÐç»/ìWPowerLawTXS 0815-094?ïöÐüSÅq?QaoÌ`ª?R^:8t?QaoÌ`ª?ïs­…Îzf?")•z¦r?'ŠOBÁM?")•z¦r?ï©ð̱I?ƒ=•-ïg…?…ƒÌál,~?ƒ=•-ïg…?5ß?MLlEʤ?§"¤ŽZÅ?MLlEʤ?ïܖѾ#<?k«&µ"˜{?q´—q'D?k«&µ"˜{?ëT»£Ú/?Ã6PìN×?­p•¿D?Ã6PìN×?îðuJ#?˜œ ‰AŎ? ÷(¬KÁØ?˜œ ‰AŎ?ç,?#+~?°|ˆés!?Ñõ§¹©?°|ˆés!AGN3FGL J0818.2+4223@fFˆ?Õ%@@³YLVÀ7a{E¼À:Ú;2Ûõ_?öÞÙ|ˆ'´@›:Ö@?ÿŠx»}š¿ß 0öܯˆ¿á~ñ`°+¿á"t˜¼¿¿æëÓ=)V;AGNbll@ƒÓ–R½<6LogParabolaS4 0814+42?ïþɶ0ÂÚ?Ò'<&r?#dŸ-ò
?Ò'<&r?ï¿Ç3ìÒ¸?ˆÇêj
˜‡?€3
¢¨?ˆÇêj
˜‡?ïÁÕßE?€"KÏÙÊ?EËqD?€"KÏÙÊ?ï-^ÕÎS5?|LkÄûo?šT%D}Ël?|LkÄûo?ïú³²s?Feìòõ¾þ?E3ô£jÁ?Feìòõ¾þ?îµHÌD?«çð—;Í4?¤®+~·T»?«çð—;Í4?ï'jZp ?º´Qu?‹ez_?º´Qu?í—tˆ4ŽÊ? ¨(óQ6x?³D[¾[‰­? ¨(óQ6xAGN3FGL J0818.8+2751@h_™÷L@>e;?q/À:30'8'À;ã:ÆG¿ÝS!@	«l'¥^Ÿ@´Þ?ä"¿ãÕgš1Þ¹¿èÓ÷4¬Û¿×ö´·Ø¿ïÿÙÍ|[AGNbll@ˆ²;Í5¨XPowerLaw5C 07.119?ï׸<Jï?­'Mõò¯?t#áüÊÄq?­'Mõò¯?ïÉm-™°?"ûFÚE`{?{Ii&z<?"ûFÚE`{?'±jh?"¬IM¶?¤æÔéY~?"¬IM¶?ï‡LÔ*Jh?z"×EF:2?Ž,ÊîŽ.%?z"×EF:2?ïùEî™?aw植á#?Kšé	ÞՏ?aw植á#?í.G™ÅX?À"Õ!É?¶Ã6³á½?À"Õ!É?Yon?Ÿ&ÓJ➾?§?¤Êi	?Ÿ&ÓJ➾?è2Ò®Ê>Ž?Àø¡D']?Ï4µD×Ç?Àø¡D']AGN3FGL J0820.4+3640@g Á¿½ð'@@pÀOæÈÀ:³Ô®BžÀ;ã·N¶Fy¿ø~&¡l@Ž£?µ¢@Cà{Ö:¿Ü:®%•¿çk	¶©û¿âÑbk/#¿àIq	úÍAGNbll@"~ËxFÜPowerLawMG2 J082018+3640?ïÿ—NT•?
ý˜eÍ{é?
,b?Âû?
ý˜eÍ{é?ïߍõ4S?!Àcl¿Ñ?p9y÷§fÃ?!Àcl¿Ñ?ïãF/~¸?e3-´ƒ&Ô?l¹Ð—ñǃ?e3-´ƒ&Ô?ïÿÙeG¾—>ê29^ü~>óM:ÕJÛ>ê29^ü~?ïþêÛok·?$¦Á¢EÛ?!RH(÷£R?$¦Á¢EÛ?ïIæѹNH?«õG˜°?–Ã%ÈÖ6ó?«õG˜°?ïŽÃüˆk
?–BÀýˆB?ŒOäÄtÀ?–BÀýˆB?ïû¦†‰hì?AØo3Öæ?Aeæ!ÛL?AØo3ÖæAGN3FGL J0820.9-1258@mfbŸœèÙ@*SŒÿWc"À:w "@ºÀ;·+rt'¢¿òzí¿`¨Œ@€â¦Rå€@,Ó P—ó¿êâ=‹Ä¿ây'vg¿ÜõF""ð¦¿æh¾òæß?AGNbll@fóœ¾àPowerLawPKS 0818-128?ïþíCÉ{? }"öwÄ+?!/ÜÅx£? }"öwÄ+?ïЖ?"aï?‡`P¢¯ÂÑ?w´à-ø·?‡`P¢¯ÂÑ?ïÞÐGN?hÃ+R…C?p—ù¥­­?hÃ+R…C?ïÿ…rVoß?´ª•ù?£mgrûp?´ª•ù?ïùVš¸ÊÚ?MFFï_Œ?J¥•›Òõ‰?MFFï_Œ?ïC†Úû
Ó?¡LË¡ã?—$ žE¦?¡LË¡ã?ïeÙ²¨"7?"*šÐ?"DÉ¢d³"?"*šÐ?ïø)m^?J!L(¥´Ã?OZLzáx?J!L(¥´ÃAGN3FGL J0822.6-4250e@pE•:À
5ðŸºÅäÀ7A9†3‹À:H{$cŒ—?ñÏoÏpÁ@}3¤GG'@iº?V'¿ÉŽ;l'¥¿ã3݆Xt¿ßŠRiY_î¿âýŠoZ*ïOTHERSNR@¡Ÿî—OßPowerLawPuppis A?è쎺~§·?ÉblÂÝ
?ÌMÅa$?ÉblÂÝ
?é—òî8q?Ãq¤ˆ
%?É¢4G;?Ãq¤ˆ
%?çFP!^'0?´Åa²¼?Ñs_½C±Ÿ?´Åa²¼?é،¼'ô?¦!=Á›Z(?ȝͽ¸2?¦!=Á›Z(?á[»K´Î?ν4ž1?ÝH‰h–cÒ?ν4ž1?Ñ6$	–ú?Ç¡'©"‰Ô?çdÿíû4ƒ?Ç¡'©"‰Ô?æè7½¢?´­*9?Ò/'â"Þ»?´­*9?Ù«hŠ>C?¸ÐôÙï¼?ã*KºàÞt?¸ÐôÙï¼MIXED3FGL J0822.9+4041@fŒ8¾øγ@A`	UÀ9Ê";ÝÀ;¯ÌÐþŠµ¿ß®Õ'[°ø@©F>RÌ@éà‰¿ä—ìëÑì¿å¾Ó¨'·¬¿êîCe'¿ÑÌÎû%OÆAGNfsrq@‹5ÜÆ?PowerLawB3 0819+408?ïÿÕ]óƒÎ>ùp8¿6\>õPþǕå1>ùp8¿6\?ïÙ·"U?…m>3ü¸¡?s$x^yE±?…m>3ü¸¡?ïå?™aÕ!?^÷|+Õ/ð?jÀfŸŠ·?^÷|+Õ/ð?ïÿsOz^?™óX—?–o\ñ^?™óX—?ïÿÁ¹£Ù?*DäaZÉ>ÿv	į¢?*DäaZÉ?ïUw3pÎR?¢¯C}lã?•Q‰O/Ï?¢¯C}lã?ïÑ'v‰?vÙDz'jC?wl|¸\Ý7?vÙDz'jC?ï÷¬½ôÓã?M+tÃ8?P¦ƒÆ¡J?M+tÃ8AGN3FGL J0824.1+2434@hàéߗª¬@>Šô PmÀ9Í]®1À;¬'Ä"Bh¿®U;¾˜Û@I¯K‡"@$e –"—¿änǬZ/¿ç	®éî¿å—÷9v²ÿ¿å°¾Õ˜AGNfsrq@‰S™0¾
íPowerLawB2 0821+24?ïÿ"m4á´?FÞw7…?
ä¤â¹?FÞw7…?ï×Ù0ïrO?ƒ}†W?tg†çP?ƒ}†W?ïì_r½rù?YÓzÁQ?c q?\?YÓzÁQ?ïôâ÷ËA÷?:pªmå¡~?V:P¾â?:pªmå¡~?ïÿ"0<Äé?ÔЗ8N?¹û/Þ·/?ÔЗ8N?ï<|@©y?¢áI÷
öµ?˜pwïø6b?¢áI÷
öµ?ïØî
gÁ?t8«øSÔ·?sð‰/®?t8«øSÔ·?ï|n%!¢'?€2"1<çQ?r;[Ë­¾?€2"1<çQAGN3FGL J0824.9+5551@d?n «†@A'Ÿ¸—ŒÀ98cϳ1À;ÑF2ê8?Á ¸è®@¢é¹íw@ÙÃߓMû¿ã\<´š¿ê^+œ;¿ä²67ìÍÁ¿é—ÐAGNfsrq@~*.Hè§PowerLawOJ 535?ïÿr£­æû?Ö»èø†?«Žø15Y?Ö»èø†?ïÚ4d
Áz?"ëé9?råÍñ°G?"ëé9?ïà"Ý(JÞ?cRsu±ž?ol#¹¬?cRsu±ž?ïþ$»$?3MéKäÃ?/M¸'Äí·?3MéKäÃ?ïÿÀ¢rV>úÌnÅÄèÄ>ÿ®¾3J›q>úÌnÅÄèÄ?ïJ"–…Ƈ?«Mƒ©]Õö?–¯m4n™&?«Mƒ©]Õö?ïÝtw°î?v©®Œà?qEÄZ
?v©®Œà?ïõ;'")ù?MpˆwMz?UˆÝ
éÝ9?MpˆwMzAGN3FGL J0824.9+3916@fį_Ô{î@AU_­åÀ9Ć4b\À;Õ½5?âm¸¼Êv@jŠ'T@>`
ø¿èžŠçq‹¿ÝZ"e'¿è(ð@¼«¿ïÿà­Õ:ÚAGNfsrq@ˆé‹]ÌcñPowerLaw4C +39.23?ïÓ}à¢äé?€³šGþ•?vA¤î£k?€³šGþ•?ïº_j|S@?‡'Ø؋×@?h%grqä?‡'Ø؋×@?ìͱΤ(?¦GȾ…?¹'qŽæ÷Á?¦GȾ…?îâç×ÑHï?{pŒ
²j?¡Ñ'†[
?{pŒ
²j?ï–+…Ù?éÝ·p‰?Š~5,`ì?éÝ·p‰?íÏBFæ2=?²Q·eƒþ­?±…íÉ<a•?²Q·eƒþ­?딄H›ò‡?°,‹Þ…?Á­îݐ5å?°,‹Þ…?æ´	 £à+?°ÞÄی7?җ쾸?«?°ÞÄی7AGN3FGL J0825.4-0213@lFÔà—"ì@3®Û@-¹À:S¤A"HGÀ;Ïçû&|l¿¸Åb$Lm@	2Á濽@5œŸ]}ß¿ç\ÄfZ6¿ä7;‰ªˆ¿æpÇNaÖ¿æƉ"ßgÑAGNbcu@
{žäPowerLawPMN J0825-0204?ïû8üuÝ?Sűpøì?C§}ÚR?Sűpøì?ï¶òãaä¡?‡M\ü›¡¦?'CG ]³?‡M\ü›¡¦?ïU_ã•f.?dÛǝ€1?•T‰ãž>?dÛǝ€1?ï1>`…HK?eÿãx´?™Ø3òƒ"?eÿãx´?ïÓjð'´"?€Jòþ ë"?vJˆr
?€Jòþ ë"?êPasÚº™?É2Y2e?ƾz0•ž?É2Y2e?îÑ@ÏÓè?¢«Mö'ðý?®âëò&Ú}?¢«Mö'ðý?âµVfǒÚ?ÁH1i{æù?ڕS2pÚM?ÁH1i{æùAGN3FGL J0825.8-3217@o"Àh¡@
i¿ÿ´ÖŒÀ9d8Ž¼ÇÀ;Z|¼A%¿ýÿÈØK†@{ âù‰ï@ê®YÒY¿çq¼*	¶/¿äó®é¿ä§Úb{d¿êk…xêAGNbcu@…]Þ҈ÎpPowerLawPKS 0823-321?ïûòŒ¤é"?@Ó¶y?¹?@5ÌçÜ4L?@Ó¶y?¹?￘,˜J ?Šxf¨‡qo?€ôÝ´éé?Šxf¨‡qo?ï†(U+"?‰€*ÇN¿ž?Žuêµ7|;?‰€*ÇN¿ž?ïÿÿ^ðP`>ßjŠ¹©>""±Í}Vø>ßjŠ¹©?ïúŸýДœ?G7Y_L(¾?E€	y%
¦?G7Y_L(¾?îƒþ•ám?²d½º
Ri?§Ï€¡é0?²d½º
Ri?îZîG¾'?¡‡w.úý?ªQ"?¡‡w.úý?ïÿùĸ'>Ïϕ54	S>˓ì~Ü1k>Ïϕ54	SAGN3FGL J0825.9-2230@n~à°¯`@!Ùäúœ>À7ŸA¥ÃtÀ:Èï'j¨?çÏ™à@4%죬Ã@cÀCÒh¿Û‡y§Çëοâè$Zìú¿ÞíñN{'¿Ý>"[U!AGNbll@"|@IQƒPowerLawPKS 0823-223?ïÿ‡Úäµ? ãâÑo?9Å7 ¿? ãâÑo?»tpü?Nék?ÉW?‡''-2"Ý?Nék?ÉW?ïކÿÊ6V?wõBŸ¥J?p¼€ÅM)?wõBŸ¥J?ïÖé
þ£è?Ylù
iü£?t‹xãÑT&?Ylù
iü£?ïþlßsºÚ?(È.
C¨@?)2æÂâÖ?(È.
C¨@?î¹Ï¼b¿?¼S6*Uá?¯"c¦?¼S6*Uá?ï°ârŒ¡?<ôåá?ƒýUžgì?<ôåá?ïAëjÐ6?†Ý'@{_?—Â'§±0?†Ý'@{_AGN3FGL J0826.0+0307@k¨ø -à@6mÀÊ`À9Ýa…V¶À;¬½D¦"¿ìïAïíö@ 2)gW@<Çÿ]˜·¿äàÿÆì…q¿áT'8§;n¿×ô'ª,¿ã)ç/#¯AGNbll@¡"vE¡ÊÁPowerLawPKS 0823+033?ïÿŠÁ±Þ?F£Ôl?
Oœ]"¾?F£Ôl?ïԌÐ+Ð?"¥¬ùýðL?u¹˜	$?"¥¬ùýðL?ïõ?ïs?^
—Ûç‡?U÷€pÐè?^
—Ûç‡?ïÿˆˆ#7>ý<ÙìsŠ?
Ýò{:±ä>ý<ÙìsŠ?ïÿh@ŽÄ?p@ZûÃ$?÷îø±y?p@ZûÃ$?ï#³¦vª?­šqúÿ?›‰Ÿë1*´?­šqúÿ?ïó©§ÑD?d'I+֒/?X¬°hæ7ö?d'I+֒/?ïúèÛeÖ??B—åâÓO?D\"~Üf??B—åâÓOAGN3FGL J0827.2-0711@lޛ6†¥@1Š	cr–À9ë:^ ŸGÀ;²ÔG'‡¿	äÐçž@
j°ëoÐ@‰žŸgäÁ¿ÞÔl´Z¿è~{å˜d¿ÎƒÉÈò‰¿ÙD÷}$™AGNbcu@¡¦Zû~'PowerLawPMN J0827-0708?ïÿb`ÐÙ?'hâ•ï?³¯•ü"?'hâ•ï?ïÅãµ$B2?}Ét÷¥s?}%i¿^í?}Ét÷¥s?ïÙ͔{€2?v8nfÀ?s5ÄO«/?v8nfÀ?ïò¶u"Îü?AJÆùR¬?Z"RqÐ?AJÆùR¬?ïüñÿæ?:í1f>4?8sŽJ@Û?:í1f>4?îüž4±\?¦ù°Ÿ²? 6ÁˆŸA?¦ù°Ÿ²?ïÎ:ÞÖÃ#?'åÒΊº?x␣¼¶<?'åÒΊº?ùƒ¦?^î}¶?‹ÙÁ¢®2†?^î}¶AGN3FGL J0828.5+5217@dʽQï·@Aã(CìÀ:ÊÐþŠ´úÀ<!‰X¿ºáӞf÷ @g¤Ôá@'¿ãZX¿ëê)1°.å¿Ö6¯¿ÔOÙìðڿ당Šá×AGNfsrq@ o¡$Ý/PowerLawTXS 0824+524?îý•Põ?±³œ½7(? &«ÏLª?±³œ½7(?ïÌ£ £[?ˆŠŸük=>?y®o¨Ó?ˆŠŸük=>?ì›mè¡û¤?«$µNÓc?»$ºð"à?«$µNÓc?ï¾ôbú}?g•;˜áÔ?€Bç>¾°Ã?g•;˜áÔ?ì×À¤S?ÂqßK)Ÿ?¿ÁAúÝg‹?ÂqßK)Ÿ?ä>_?² °º›í?¦wA¼ú!
?² °º›í?ê Ì‰Ž'2?¸ïÁ¤Ë]?Å|ÍÙÅ·7?¸ïÁ¤Ë]?í—Íf¥¦?¬Ï©Aék?·ûA•¦¹Ë?¬Ï©AékAGN3FGL J0828.8-2420@n¼WÀ±5˜@ Õ¶`#× À:6ÄíÛ:NÀ;±Ø{V¸¿æP˜#Lá/@
Ū‰€ò¯?ÿþ½?'‡¿ÒLS'ÿ¿é×:$ȿȏcüï2¿ãˆŒ£^aAGNbcu@©Éçü¹#£PowerLawNVSS J082841-241850?ïþýÉÄڐ?!·!ÄLdˆ? #eÂüä?!·!ÄLdˆ?ï²¼Û#c?"z,øζÆ?ƒyÓÝñ6?"z,øζÆ?ï׳³KFz?wqúŽ'²?t&&_,6È?wqúŽ'²?ïþb]dž?tËÓÿM?)ß{
mXQ?tËÓÿM?ïý˼ù½h?2%i¿Ž9?1¢%ÌÙü?2%i¿Ž9?îXŒe æ?·ê
mòcð?ªw9¦Í†G?·ê
mòcð?ïڃìU "?wzX7?r¾	àÞb†?wzX7?ïðÞÍ*j¸?VKH@G+*?^Beܤð^?VKH@G+*AGN3FGL J0829.3+0901@jý؈v\@9ÓÉ¿Ò‡À:¨L…ЗÀ;à\KZqf?Þv~;U}@c‡'ÛåD?ÿ(ÜP'`¿ïÿÕYu?ïýv8t^¿àò±C÷.¿Ô÷P0;~~AGNfsrq@¨¹sœ¾àPowerLawTXS 0826+091?ïþeåHTê?&¦MJ\ë[?)¡ª!rAQ?&¦MJ\ë[?ïµÄc*r?ˆøP\"}b?'ŽÜ·³ƒx?ˆøP\"}b?ïÒ­üŸo¿?m2mG¤ò?v©Ž›ôÉ?m2mG¤ò?ï8BO–ýC?€{¬%¼ÂÞ?˜÷¶Ø%•?€{¬%¼ÂÞ?ïù-ëmT?G™—‰øË©?KHQÉà¥:?G™—‰øË©?í"l'ùÞÃ?¹W÷‹šÛí?¶ì›ézäj?¹W÷‹šÛí?ï•>¡ây™?…l(zÑ
'?Š°WŽ@ÑÖ?…l(zÑ
'?éw*Ý?¶Ûe"?Ê#T‹ûÿÉ?¶Ûe"AGN3FGL J0829.6-1137@mf[ ¥&–@/\7 þ}IÀ:SÐ-hïÀ;¿ŸàÛwŠ¿õb ¼8*@AåÀ8À?þ;Úß_ ¢¿Ê±¡NU	¿ìF»,Þ§¸?Ñ~°ŸšŽ¿Ôr¨©ïAGNbcu@®ëaÊÀƒPowerLawNVSS J082939-114103?ïÿwy*°¥?`FPo¶?Ù7)ÿà?`FPo¶?ïӓzñÌ?"‰º"Á±?v6Bt«5ì?"‰º"Á±?ïæ:ðI‡;?pgƒ"âž?iÅÈV¼Á?pgƒ"âž?ïÿûõü"[>ºÑ3=¹*>À(¶§l¶c>ºÑ3=¹*?ïÿ­›¢f?•Ñõœ?¼Òö-kg?•Ñõœ?ï…@¤¾n?´E'Ä?ŸoWëh22?´E'Ä?ïé'z™#R?pìp»…ÐÛ?f}…"$~K?pìp»…ÐÛ?ïÿîœD2¤>â%ž"O¾Ó>ác""rv¢>â%ž"O¾ÓAGN3FGL J0830.3-5855@q%ˆ¿Â"OÀ&ã
F:À9Z¾ÝöÀ¼À;†aQS°?è3ˆ2˜ü@=òFƒòé@Ý»à~í¿è˜p&Œ9¿è¬-ÎFl¿äÌ~?Ã\¿ïÿ¯í1àçAGNbcu@€"4êKPowerLawPMN J0829-5856?ïû\FÄ?E	m»û™?AúŽì·aÍ?E	m»û™?ï.æÐYT?™x£AóqP?š#%ñl™z?™x£AóqP?×(?|MÑ
1ˆ?‰ÚŠ+È'?|MÑ
1ˆ?î*À-µ£n?…+éáÝ4Œ?­Sý ZF%?…+éáÝ4Œ?ïø†:'\?Q郇šÝ?Mçd×?Q郇šÝ?æå@??É¢fi7ôZ?ÓÃÝú5ƒ?É¢fi7ôZ?î¶Ö\SÏ?ž'…Qw¼±?¤'š9@N?ž'…Qw¼±?äù#»N¨¸?²ÈJåø?Ö
¸‰b®?²ÈJåøAGN3FGL J0830.7+2408@iòà\̊@?Ô· "À8¯â*ðoÀ;'çf¬"?î,Û`–÷1@è]…TÖ@í?³õ¿å@É-}^¿é6ÀNí¿çr
²©`¿ìm«ÞöAGNFSRQ@€.záHPowerLawOJ 248?ïúüê+?CšRú•\D?DXRë»c?CšRú•\D?ïÉ»Ôh2Õ?€íâ7Â_ô?{"â"#?€íâ7Â_ô?ïŒë'M*?}"=×<?Œú…)»‰Z?}"=×<?ï70ç?ue`40¡?™ÿÕ'?ue`40¡?ïúè—(?C«u¢	"ë?Gð`Kòƚ?C«u¢	"ë?îz™fmó#?°¡^hæÕT?¨Vi™ ÍÖ?°¡^hæÕT?ïxǬHë#?S)}äî?ç
q»1®?S)}äî?ëzƒˆC?§·Ò@‰oñ?ÂÝó¡Þô?§·Ò@‰oñAGN3FGL J0831.9+0430@k–Š r~@8^'ŸªTÓÀ8&–5À;9¯4^¬?ö wÔÍÍ(@*íEé]@°Ì`Á5ë¿Ú~Oû"´õ¿å
‡òÓ¿ä2z ë¿çC^ˬ*/AGNbll@€aàA‰7LLogParabolaPKS 0829+046?ïÿ'£+˜?XÎώ¤š?›RúùY?XÎώ¤š?ïÌF²¾?‡]ƒ
Èî?yܞ¨Txú?‡]ƒ
Èî?ïÅúU€?}ßA`ËÜ]?}ÿØøˆ?}ßA`ËÜ]?ïæÏ/'µÒ?M0OÓÈüÃ?i0ÐÂL®–?M0OÓÈüÃ?ïþb'ß?1M€¹ÈÖ?/™Ôʨ-?1M€¹ÈÖ?ïåHÜÀ?²c¾ÏÌ?ŸcVø›më?²c¾ÏÌ?ï…@ñ"3£?ïWS]|?Ž¯Ã©Aë"?ïWS]|?ïÉO¯•¯T?pRü°Îí?{X(@×Ï?pRü°ÎíAGN3FGL J0832.6+4914@eC[ÿW~@B6| À:¥kÏ[óFÀ<>ô1•¤¿ÑHe²¿ãä@
'žÜsß@è? ©Ù-¿ºä¸·þÝ¿é+'Ÿëñ¿àöäð§j¿çJ+í;#ºAGNbll@'¡–R½<PowerLawOJ 448?ïþ‹_]Å?0LI	íB?'Nmš»ï6?0LI	íB?ïÛp³5:ä?ƒ'D`?rG¦DfN ?ƒ'D`?ï­2¸¹ðQ?€mˆý;ÀÑ?"³QßB[Ÿ?€mˆý;ÀÑ?ïïaj ?H Æ,øA'?`øžØ·Øo?H Æ,øA'?ïú˜Öß?IC4–¤ä?Eœ§ÀIÃÛ?IC4–¤ä?î÷_Žl%(?±#"}Hm<? Š­Iu?±#"}Hm<?ïôpbq?—Lm Qʜ?}+yá?—Lm Qʜ?ïg›œ?'_G³ø?œ3¡œ(‡?'_G³øAGN3FGL J0834.1+4223@fSëßL+R@B'±ÀoÀ9f:¢"=_À;Ȍ{£åM¿ôž6ìü=@<¦Ú'Q@ƒÀ`óJ¿å«cÛi8¿ç©Á‰Å©¿ÝTPф~¿é£Ü^nAGNfsrq@ˆºáG®PowerLawOJ 451?ïûËJõ$b?=ϖ|a#K?@ÒÔPCßÄ?=ϖ|a#K?ïÛ?öÝcë?…>¡ÝR/?r`xÚ‹?…>¡ÝR/?ïÕÒ¡fÜG?q$"¾É?u¯>Ól¨?q$"¾É?ïÿB>O,I?œ¡¼?¸8¹*"²?œ¡¼?ïú·€¬°?JHjmØ-Ó?E!üýˆ«²?JHjmØ-Ó?ïP,£Lé?ªºã.L¿W?•úk™ëžÖ?ªºã.L¿W?ïpʅL??góUãçe?'æ¯b]â?góUãçe?ïð¼qœ
É?['ïvZ¦E?^‡¢?['ïvZ¦EAGN3FGL J0834.7+4403@f^Ñ·@BH{Àj¾»À:l{¯£ÇÀ<Ä3¡<À¨ˆ‹ªB´@%š_'6Ï@½:¿™ˆ}¿ê#"±*ãa¿Ïh
Ô"	H¿ä&\tŽáô¿â7ÁGˆÁAGNbll@™™Æ?PowerLawB3 0831+442?ïÿ"·‡b­? ö5r¿­?©½ˆÜ? ö5r¿­?ïà7u¯"?'yu¹º?oȊôk­?'yu¹º?ïÆ­/ge"?ƒL"ó™?|©h8_'F?ƒL"ó™?ïÿþ"c¹>¨emâ'T9>¦¾—wœ¬N>¨emâ'T9?ïþ»tŠÁe?#Iµ*7çé?$H³˜p*?#Iµ*7çé?ï]åL9X?£UÇõ±ú7?"_ÃX0¢ó?£UÇõ±ú7?ïÅy›Ä¹z?KĹÖa?}C2'òÆ?KĹÖa?ïÿÊo>@?mcápX>úÈ«JM?mcápXAGN3FGL J0835.3-4510@pxß¿ƒ8.ÀLV ž9À2ˆ©ÀXJDÀ8Çå"S·@衦ˆ›@ø9'rÞÅ?ôž£¼ˆ1¿Ð†bbÔ>¿àÝskâ¿å>¢ÔšS¿ì̋Ç0PSRPSR@Št‡ü¹$PLSuperExpCutoffPSR J0835-4510?kÝß&"(?­ŽÈ´~@?ïä" ç+H?­ŽÈ´~@?£
ր?Àuւ?îÏ/ò¥¾/?Àuւ?%˜áÏ?ã\™#¡?ïƒkõœyÉ?ã\™#¡>†8²˜\/>‡aì,ä?ïÿÿ¦á"<>‡aì,ä?%':m]¼?!ü wµ*Ì?ïþ¦Ö÷?!ü wµ*Ì?…†Ò¬/ªZ?¤³RçÃ?ï©äµG—?¤³RçÃ?|ÏuÜkŸb?'Ç×JÏ9?ïÆa[Æi?'Ç×JÏ9>OnÀ/sW]>^BßU!ã?ïÿÿ÷òjk>^BßU!ãPSR3FGL J0835.4+0930@ko?Rü&@;fi¿·:"À:WozânÀ;Ô$n:¿Â"+l=@³ieIZè@OÉ Gˆ«¿ä'Õ""¿êV_T?·¿Ñ©Îée<x¿ßoò2bAGNbll@—wu\)PowerLawGB6 J0835+0936?ïþ€ÿÍ]Ê?;q–mË?'ð¼8æ?;q–mË?ïØ'Œ$Ö?",Ž#§Ï?sÿlZ9èõ?",Ž#§Ï?ïÀS"âRp?Ðb²•}?Ö=wyp?Ðb²•}?ïî,Þ&Þ³?J®»Ì]?aÓ!ôž,c?J®»Ì]?ïûП%…Ý?G'ŽYíìC?@½ƒxÀv³?G'ŽYíìC?î´¿µë'h?¶n»ß|˜P?¤´Ÿ}?¶n»ß|˜P?ïPÊ,€ÞÚ?"{ŸÕë%ö?•æºq›ò¼?"{ŸÕë%ö?ï;ïß^\?öÅ=ô
?˜'\f?öÅ=ô
AGN3FGL J0836.3+2143@ih*Á	J,@@$ÓÀíÀ:K/ÉgeÀ;Ô¶JªH¿¥ŸtD¸{8@
†Ã(3P@†š@ˆ†L¿çZþÞdFH¿èð­&¿2¿çÙÔ5ˆ^¿Ó(^öQø¾AGNbcu@‡RÓÃa@PowerLawMG2 J083615+2138?ïÿ´‡ a¤?Ç»Jt?Þz§Fh?Ç»Jt?ïÛ9†ñT?'™²Úb€‹?rcUD…ä?'™²Úb€‹?ïãz¬L,\?løJ2·åð?l…S‰8|4?løJ2·åð?ïý˜?/'?`T[°2s?3>
:ô?`T[°2s?ïÿƒ¼É°Ÿ?R§–¨ªˆ?Ìêõ¼O?R§–¨ªˆ?ïM·#Jæa?¢ÅŸçÿg±?–I'{Éí?¢ÅŸçÿg±?ïÃƤû³¦?€d¼½=H?~­v@Þ?€d¼½=H?ïá-×Ԓ¿?e>pP¼…S?nÒ(ϙ>?e>pP¼…SAGN3FGL J0836.5-2020@nsŸ‡ð$@([qàíìÀ9"ØC""À;¢Þ"umj?Ø[·Êßõ@ - ®@Û$¼"Û¿ècpÎQ宿鞡S!e*¿é ,W™;r¿ïýÁ\‰ÌPAGNfsrq@xôNã'áïPowerLawPKS 0834-20?ïíMl´" ?`"øLÔ+?b²"*á Y?`"øLÔ+?ïrèyjhî?"Ñ+]$>?'¢ð͋x??"Ñ+]$>?ïLéÐh¸¦?…Ÿ=8í£?–bÅòèë;?…Ÿ=8í£?HËÜô?ƒ>F*Ö?¦·ûp®{Ä?ƒ>F*Ö?ïÅ]žx?zù‡(ió?}Qr²#Ò?zù‡(ió?é±SB$ñ/?ÇÍ4[|RŒ?É:²÷l;E?ÇÍ4[|RŒ?î—½»%Ê?¢ÿu߈ľ?®†"'½?X?¢ÿu߈ľ?âq‹÷">w?²ØQñ¿ip?Û軃?²ØQñ¿ipAGN3FGL J0838.1-4615@p‹ƒÀ~à±À\ `ˆ+À8$›†ãàÀ9¼n9™~Â?öű:5¥@ï†<š?ÿϾúQ?c¿Ù:E E›¿ã3õƒ¥¿éµŒ©ÇG¿î¥x?V×þOTHERspp@•åDêJŒLogParabola?Ü¿/&€k?ÑÁß÷†|?á hló?Ë?ÑÁß÷†|?ëßØù^ƒÍ?¿lÐ7æKN?À€œ…ðÎ?¿lÐ7æKN?ÚL›Þ‡#9?³"5`¿Ek?âÙ²¼nc?³"5`¿Ek?깄ò~ÉE?¡¡†ZÊa?Åì6Úì?¡¡†ZÊa?ÕAi² N)?Ì·NBO¨+?å_K&ïØë?Ì·NBO¨+?Ö¯‹³ÒÕÐ?ʍKÔ%÷?ä¨:&•?ʍKÔ%÷?à
xkQ?¿çéÖl?ßå)ÏÃ]?¿çéÖl?ÞÓ¦·¢™?º¿âà¤4?à–,¤p.´?º¿âà¤4MIXED3FGL J0839.1-4739@pžæ?šIÃÀ#Á`]öÀ9¢t3®ƒÀ:ZQU]*?ñò÷c#f@âeæ9@®èŸf7B¿ÞŒ£çÑ5¿í°˜ƒïä)¿ìZ¾b¦¾?Ç¥}=OTHERspp@™ƒOAò×PowerLaw?êÝ5À9ü?ÆÄPuý÷×?ċ(ýû?ÆÄPuý÷×?ïG$wÀÐ?¨_·u¢™s?—q#'	?¨_·u¢™s?æÀ-¦¤?·C«½$ç€?ÒÅÙ¤²¹?·C«½$ç€?ïÒÛhž?l×b>ó®?v÷'j¥?l×b>ó®?âH™cÆÃ?Ϟ‰&ž"?ÛnÍ9üry?Ϟ‰&ž"?è…5Nkrë?ÌLrÌêï?Íë*ÆR4U?ÌLrÌêï?ãjq€ÿL"?¸@Úe¼U?Ù+þf÷?¸@Úe¼U?îAG¸GÑó?­ïŒ»E?«ë"yËÐ?­ïŒ»EAGN3FGL J0839.5+0102@l!O?Ù3ã@8_L?s³VÀ9È[[piÀ;ďñz+??ò%ëú}·@<'è§HÚ@æ­àMˆ¿ºsçûž¾¿¿à‡Q¿ ¢ô¿äE|	w[¿ïÿ‹Z,$AGNfsrq@'ÑXâePowerLawPKS 0837+012?ïÄö—Ó?ƒ8鱯	?}ñ"¦:_?ƒ8鱯	?ïºE¯Î?ŒúëÐzÜ?n"¬?ŒúëÐzÜ?êElÛN?®¿ZzH;?ÇæêO"'Ê?®¿ZzH;?ïSÜ=®l?s@,ûìŒ?•"xQʃ?s@,ûìŒ?ïTøÞß°?˜â¡a{?•`ä)1h?˜â¡a{?î‹wǯ#?µWøsP?§Hƒ…éµý?µWøsP?æ4p%"»?¶Û‹ žË?ӗ´Ùċ?¶Û‹ žË?íw@_°X'?žÝŒ£ìøŸ?´Eý¢üð?žÝŒ£ìøŸAGN3FGL J0839.6+3538@gcôŸM¡@B>n¿Ñ;ÇÀ:w»"€^À;¾–ä•?ˁâmÈÛ@
íæšÔ,=?þÄl@šúÿÛijãà¿Ø)ÉMˆÁ¿Û§7á\•œ¿ã°UþdIAGNbll@¤>µ›=ÈPowerLawFIRST J083943.3+354001?ïÿšþ?/µe²8?Ÿ"H('?/µe²8?ïÏK°é¨Œ?"娏 †î?xZ'p^Æ5?"娏 †î?ïãbð‡‰n?dQ4Ϧ­?l»Îéƒ?dQ4Ϧ­?ï¹¼âu?bô¡E{?øÔI·?bô¡E{?ïûp.^?AL…ÛNµ?B?GË*'›?AL…ÛNµ?îÒ}1Ⱦº?ª¦8EU:?¢Ø,â˜-a?ª¦8EU:?ïÍÕlÈD?y|
|*©ê?yI‰P6?y|
|*©ê?íoH~¸±|? ¡Ck–zK?´…¼"N¡? ¡Ck–zKAGN3FGL J0839.6+1803@ióÿ`Ï‰@?ÁúàŽµÀ:g8Yã¡%À;Û²ìPö"¿ñ~n¸Œ@WÕé4-?þwæ Zé[?µ&Pƒ{H¿ß3pÍ?ð¿Ûÿ)w-ð¿±bÓkÄÁˆAGNbll@¬c{J#:PowerLawTXS 0836+182?ïÿpC}?‰ÌøÜå]?')Ĝ÷?‰ÌøÜå]?ïÖ@ç%ét?†9‡%Ǽw?tߌuúB#?†9‡%Ǽw?ïàÑå:'?gk{v]rT?or.NÿÛ?gk{v]rT?ïÿäÅÎ,>àÍñ8ìô>ë9ï~´.¼>àÍñ8ìô?ïþÜg@ù?1¢ê"É"?.r;=%O?1¢ê"É"?ïI\¿!?ªIّüù-?–ÌTbõñô?ªIّüù-?ïÉFÞ-??}¸éÝ&%Ì?{}\ˆªP§?}¸éÝ&%Ì?ïþwƒˆúÕ?(ŸÑâ黪?(‡É'®K9?(ŸÑâ黪AGN3FGL J0840.8+1315@j›Ÿ˜·@>+?8$4À9¢Àøƒ3ýÀ;À
éh?ëz¿Ôäì@9Ua0r@¾Í­ð>¿â5JBï>¿èy$ÞÔÿⴛ<Ú«¿ïÿ¸ÕҍŠAGNssrq@ƒñ	¿œb¢PowerLaw3C 207?ïÿy`Ò!?Ÿm^˅o?ÔÞ_Gï?Ÿm^˅o?ïÄ
7€8¹?‡"¸›nYE?}úä"Vÿ…?‡"¸›nYE?ï¢wýγ"?vë[üÕ§?‡b{%Y?vë[üÕ§?ïX%"Ôd?oYe~4eo?"û[µÆ;‡?oYe~4eo?ïÿ‹8‹j?Lu¨Y!??9È¥CŠ?Lu¨Y!??îÃthÿë?«×=iÏ?£Îè½»"G?«×=iÏ?ïEã#Üý?"UÆCf'?—C›—<öj?"UÆCf'?ìž?if:?¢û֑Ñáû?»æ´Î1?¢û֑ÑáûAGN3FGL J0841.3-3554@p
Ձ¥‡@
æ1ÀAyÀ8 TS>kvÀ:ðÓu]z/?òã(­"÷@tpȕ?ü:¿ë½Ô¿×¿¿¸èz¿Ö'´ƒ]v¿Ê`P¶6¿ÜòàèbªoAGNbcu@±'5`A‰7PowerLawNVSS J084121-355506?ïÚÝÓý?¾"¯ÕMØ?‰H‡'?¾"¯ÕMØ?ï@w¥¼
? o™Fá±x?—ñ]°»? o™Fá±x? 0ˆD?ŠL_² ¯@?Ž•·ðnRô?ŠL_² ¯@?ï4¡È<DT?q¦á;¨Òd?™kÆõه?q¦á;¨Òd?ïùMr¾R?NÇñ.¢?KšË#Þ?NÇñ.¢?éw;G¡ Ä?Éó½°îu?Ê#á{|ð?Éó½°îu?ï~éætO? ½IS~?<¾
)? ½IS~?íÜ?vëø??–ª¯ƒ ?±Fèp?–ª¯ƒ AGN3FGL J0841.4+7053@añ'à@A7E AYÀ8	³;+O9À;€æàtI~?ûÈ=ägF@i•šÜe@<ѯµÄ¿æ›BŒÓŸ¿ëŸÏW…g¿ëƏ¨Ì^à¿ëÆl:]@oAGNFSRQ@m‡§æšÔLogParabolaS5 0836+71?ïð-Ùö<?aX£/m?_¥À™'¿?aX£/m?ïסf‡B?'ÌЍׅ—?t/Lõ­:é?'ÌЍׅ—?í=Uë'Uu?¤£u·"|¾?¶P¥-"W?¤£u·"|¾?ïùír<f?5X°ҋ?HJ6MpΦ?5X°ҋ?ïîՌcü?c)\—õói?aø*~šÃó?c)\—õói?ï;l{@?¦À&9§K?˜'p¤e¢?¦À&9§K?íl'gŠÂ€?§b[ù¡?´›tÂ`'?§b[ù¡?ï÷Î0'²U?N™›ßÿ`q?Pcž¥el?N™›ßÿ`qAGN3FGL J0842.0-6055@qN9¿ß~€À&Ð[À6ãÀ9	füŽ[xÀ;z³Z4ÿ¼?ñ0èóžó¡@¾Ù>Js@ŸÑÀ§zƒ¿ã'»¢Fֿ嵊ÂÕìË¿àé4ü®^D¿í#ÞùÂqAGNbcu@‹ÔEÁ?ÐÐPowerLawPMN J0842-6053?ïâGáýÛ?g"•ƒñü?m¸çgDí?g"•ƒñü?îNë5¹Û?©ëúù"?«L­¨{Q?©ëúù"?z殩?•Äªw3ÿf?¥'ˆP¹.t?•Äªw3ÿf?ìê2úºW?ŽbþwË°Æ?¸®h)Q`"?ŽbþwË°Æ?ï•r¶Å"?ˆè5M•?Š¹cGÿÇA?ˆè5M•?á¤ÀÞEßÍ?ʉÆã?ܶ~Ct@f?ʉÆã?ìšf²£?¨n=?»/ÌÊjê?¨n=?ãwE4Æ?³"€•ÿ•©?ÙÙu–sä?³"€•ÿ•©AGN3FGL J0843.1-4546@pÏ`Z³«À{=ŸrÌ{À8¶Ôš÷g«À9ïg ù	l¿òŸXj¥:b@Í­ð>@D5¿æ+Å`qÚ¹¿é8"ѳ¼[¿ét5A*l»¿ÝrFnyZOTHERspp@«Ãý¿HÌPowerLaw?Ú͔Ï@«¨?ÒT»üùmó?â™5˜_ª,?ÒT»üùmó?XÖʖ?˜k(Þi®û?‡Zéͼöf?˜k(Þi®û?ákÛ@‹"û?·«²wV?Ý(I~èØ
?·«²wV?ïÿÖiP>óKvi`!>ôËeØX–Ä>óKvi`!?߸&öA˜Ú?Ïþ°r°L?à#ì"ß3"?Ïþ°r°L?í2R£o?Á¼.{àÃq?¶o×㳎?Á¼.{àÃq?ã#úGy€?ºÕÛO'°?Ù¸×q
?ºÕÛO'°?ïýe–W?5xHØñÚ?7|Ó)¿?5xHØñÚMIXED3FGL J0843.9+5311@d¢KZS3@CÒ_³Ä¾À:è>BZîÀ<‡ªƒÍ?¥sÀìa@UÍÕ
ˆð@ëõƒ¥¿æM¤_è•M¿ã‡:]N*¿Ú åÓ¾
¿ïÿ<!H"AGNbll@"F*™0¾PowerLawNVSS J084411+531250?ïîuH×_M?_ÔQ~ø®?aŠ·#!S?_ÔQ~ø®?ïϒD¥n?€ãZ¤'–?x6þy*(í?€ãZ¤'–?îõŠõÖ ?–…¸!€>?§ §NêÈ?–…¸!€>?ïp HpÌ?w‰m1EÅ?'ëý¶ñæ"?w‰m1EÅ?ïªBÊ2œ=?Šq¡Ýÿ²Ð?…oMi
É?Šq¡Ýÿ²Ð?íø­õµèô?µÊý™WÙ?°:P˜ê_?µÊý™WÙ?ëÑÞó¢?°:<½¥±c?À¸"3‰wì?°:<½¥±c?éÛéCêªG?µy—nç¬\?ȐZðUVã?µy—nç¬\AGN3FGL J0845.1-5458@qT@(äüÀéá€8ªÀ8µ|N/8À;G^X?éˆu¥@X8ü÷@[=ŸrÌ{¿ávý¨À[®¿å»ÒÿŒ¿á€o$Ç8¿éñd—ëTÞAGNbcu@2€uMPowerLawPMN J0845-5458?ï‹3˜ïá¶?"-`M'Ë?3²Ù†š?"-`M'Ë?ç‡úþ8£?ÈíQt]?Ðð
¹?ÈíQt]?î›ÿàþæƒ?š90D¸¹?¦@ëÆÕ?š90D¸¹?èH'7[?¥æî3²‡?ÎÝ»"'‹"?¥æî3²‡?ê¨-žHÕÝ?À…™çн?Å_I†Ü¨?À…™çн?ÆML€¥ò?ÇÁyõóV?êl¸ìßք?ÇÁyõóV?çÙe:Rm?´ãÛQô4?ÐM5‹ZÅ&?´ãÛQô4?ÊË*Lý>?ª³ADõ¦«?éM5lÀ¿ñ?ª³ADõ¦«MIXED3FGL J0846.7-0651@m,xßzN{@5Φ ™@À:©-‹S†À;Ãý…Ò<x¿‹GÿFô+@	 ¼c1@Ò[ßú¦û¿ävÿ¨r¿çêIf~u¿ç"Öì‹Y¿ïûõ-Wë¾AGNbll@þu%FPowerLawTXS 0845-068?ï÷
ýX­?UR3xXNq?Qêï
•×?UR3xXNq?ïÏ`i2"É?|Ž.<
•®?xOËj-7Ÿ?|Ž.<
•®?ïuÛH‡û"?|~0f‹Œ?'D–÷—•w?|~0f‹Œ?šM˜?pXìPƒÏ¦?Œ™‰;n?pXìPƒÏ¦?ïî
iæM§?cÙó³ŒÑ?aõ–=nH|?cÙó³ŒÑ?î	GîÅß·?µ}ž+ó¦?¯k2h?µ}ž+ó¦?ï<"Þ&fq?'Œuû¡û?˜{¤7Õà?'Œuû¡û?é€F¾D7¬?±uã?¬•?Éþåï!O?±uã?¬•AGN3FGL J0846.9-2336@nøeÿ£¹®@(i'¿°"˜À9	åQþÐUÀ;VZU¶ëº¿ä@$ýTBç@¯ôüåš@6ãtt¿â@")N>¿àö¸dq)õ¿ãÅ1˜±ð±¿·eÖÞôl¤AGNbll@EGÈK]ÌPowerLawPMN J0847-2337?ïþ5hÓº8?!Z¦d?,©v÷¯š?!Z¦d?ïς¿b€ÿ?"¦Y>·U)?x> B`èÅ?"¦Y>·U)?ïìb&:Ò9?_[¤œO'?cÙÝêöë?_[¤œO'?ïÿŒmF/>þýÿ3¸P?ä»p}ñ‡>þýÿ3¸P?ïý…b'*ñ?/E/)D‡f?3ÔíøS?/E/)D‡f?îÖ£L»?´c?'x¹?¢•Ë:ÈË-?´c?'x¹?ï´.qò$?ˆ':£â?G?'ôc}GM?ˆ':£â?G?ïùrw
J
?E­úo"4¢?J6#Cš`l?E­úo"4¢AGN3FGL J0847.1+1134@jî4 ½@>à•¿ðExÀ9¾Ñk—þÀ;x}›ö¿î|"eÞ^Î@oS"ºd?û؅_¥×ë?ïÍå=Sj¿Øg½¯ß']¿×ÑåÙkÊ1¿Ð'oO²ß€AGNbll@±ßÈâe,PowerLawRX J0847.1+1133?ïþI0—ïÃ?+d½9˳?+lö¼cz=?+d½9˳?ïÔ03×ü^?‰©ªÙ7?uçåóµ|ù?‰©ªÙ7?ïբ͆k?sœ»ê~È?u.™CÔ[?sœ»ê~È?ïÿ"­¡Ž[>þÓl>j¼´?
ԞEhB>þÓl>j¼´?ïûYo)zð??2f†?¹?BšD#Öèw??2f†?¹?ï8|o?ª³«êüy?˜ðr—ˆ?ª³«êüy?ïµb+²û?'ï«ðÆh?'º§wzû<?'ï«ðÆh?ïû•ýOC?>H¹Cô´?A¨¬-?>H¹Cô´AGN3FGL J0849.1+6607@bY_í¦a@B8y@]¾!À9Ô"Nßa$À;ØgÕÒ/?ÄíSÜ\H@ä'áqI™@!ŸàZž¿Ú)ÙuÛ,¿á™ ù;Ò¿Ò"¦wgYo¿çáMž™AGNbll@¢Ezxl"PowerLawGB6 J0848+6605?ïÿ!#d+?àªHt%?ܵuÆNí?àªHt%?ïß'èH˘?zªɳU?plög'½?zªɳU?ïêS6ø~p?rwîs?e¬ÈÚ&¸?rwîs?ïê
Ò/Ñï?K}@A{?eõ-Çï}?K}@A{?ïþ=L½.?.séô' Ï?,/ýÁI?ä?.séô' Ï?ïdìz8?¬'ò2þS.?œóbƒoñ?¬'ò2þS.?ïÑdQ
cÁ?€ecÙ,¥O?wM×hÏÿµ?€ecÙ,¥O?ïw
†.
ˆ?'ëB±%?'O8†á?'ëB±%AGN3FGL J0849.3+0458@kÏÿšÏú@<hÿƒ~À9Ùé¿KÛÀ;£Ö™Õ(¼¿Ì¬s"é@CŒxsÚ?ÿƒ3Ù'?ïÙ]KW
пãCUˆPN«¿ÚJ,Qº¿Ý]4wð–DAGNbll@¢Î'ÃÉîÌPowerLawTXS 0846+051?ïþ½ÆR<ì?$ï:*L¸æ?$#¯«Ä?$ï:*L¸æ?ïÒ+';<¨?Š#þ5EIE?vê6ì"×?Š#þ5EIE?ïßLœ™[å?g-ëk®?pY±»'š?g-ëk®?ïö§ãD™ž?>­?SÕý'?R°9•	Sq?>­?SÕý'?ïûÿ'=Å?Aö°ÔDe?@bn!Cª?Aö°ÔDe?ïÜuÑT?¯^ÂÝÓ?œ$qD(?¯^ÂÝÓ?ï¿QHî?€ 8\Lc?€+ºoZ\i?€ 8\Lc?ï±ÛŒO¦~?xWS5H—?ƒ‰á ›?xWS5H—AGN3FGL J0849.5-2912@o"
ŸS @"vï`¥bÀ9†°>÷Œ"À;":]Éß³?ÙÉü	È£@-Æ	99²@ñ¿€3-¿âw"©Կ㆖O7JÅ¿Ö֙qM¬¿åÿ¥2AGNbcu@›OÆÂ&€PowerLawNVSS J084922-291149?ïý:@¡8}?6<©\ùpw?6-ùŸ/æÃ?6<©\ùpw?ïžÐU‰Š?O¬u\˜?ˆK꽍9›?O¬u\˜?ïæíìs†?`«Þ˜?i'¡?`«Þ˜?ô%ù†?hkò됀?ŒÃÐrd?hkò됀?ïñG%A"?`f1?A¤/?]qÔ2‡"?`f1?A¤/?ìÂû%-i£?¿sS숡F?¹è&֔²æ?¿sS숡F?ﰝ3×óÇ?†ž"|¿±?ƒØ³
'?†ž"|¿±?ì֏r"	K? '¾Vx?¹K"kÕ©$? '¾VxAGN3FGL J0849.9-3540@pTÀ%@ùJŸ¶i3À8ýJh˜À;9©y
­Ù?äϳ?'@äSV>P@÷«ßla¨¿ã߃<yDZ¿áаd6`d¿èÌÕ÷vw3¿å%¡8/­~AGNbcu@™¯·éPowerLawPMN J0849-3541?ïþg½Íx?*ê¬ÿÆ£!?)Ž!¬	Þ¸?*ê¬ÿÆ£!?ï§V±› ¶?"&"ûeŠ ?†*SªeÞp?"&"ûeŠ ?ïµ!mk›ã?y±¯ûÞÅ·?'·¤¬P57?y±¯ûÞÅ·?ïëÛ"-°?Dºÿ>Ñi?dï$ñö?Dºÿ>Ñi?ïퟯwO?daB¼pd¾?b`P‹ª`ñ?daB¼pd¾?í¨'#ãè{?¿ëéá½?²¾ÆàÕ*?¿ëéá½?îè'BdŒ?"þti?¡vëÛæC?"þti?ï'^[¢_ˆ?|áSû~]Í?hi×¹é?|áSû~]ÍAGN3FGL J0849.9+5108@dóM@$³>@C‹ßœ³*À8…JÿÓ?À;"2¨É¸E?ð;çҌªH@'øyxçÈ@Bsàwy‰¿áJÈ|ÊÅ¥¿ä"W¿â+}Aý®õ¿ìéº~wAGNNLSY1@†KàÞ҉PowerLawSBS 0846+513?ïógÌu—?U–h$í [?Y0fÍY«?U–h$í [?ïߛhü˜Â?2–ˆ²®?p2K"A'º?2–ˆ²®?îÍj²Y¾?–B·uý§?£)Tٓ])?–B·uý§?ïÿ,'-Ûõ?ù¤iúÅæ?o»÷érê?ù¤iúÅæ?ïí¶®A5C?b<º%—G'?bIQ¶‹¬Ä?b<º%—G'?ï? ¹€a1?­RCi˜<P?˜èÓcuã?­RCi˜<P?í_ì3?¤¶löéÏê?µ7nx¥û?¤¶löéÏê?ïþ×ÃÃ08?!±®oW?"ƒÀ‹ŽrÑ?!±®oWAGN3FGL J0850.0+4855@eNù?ò^W@C£ïÿ×¼À8hìt2À;oÓ £äv?êxÛ¯iœ@Æûþ¿ö@vž_|s¿áœej¬¶¿âå0
ö¿åB™OœËR¿ã8íÉéåÚAGNbll@ŠOò×sPowerLawGB6 J0850+4855@?ïÿæ÷‡?!q )ùG-?£7‡À¦?!q )ùG-?ïâˆ(‹˜?x"ÞÕNV?mw×Ræh?x"ÞÕNV?燐ìMVÜ?…ûÂ‡‡?†DÞëÙ?…ûÂ‡‡?ïü›*­"?!ž@VÀáy?;&«èØ:œ?!ž@VÀáy?ïþ¬_]ÍT?(™¼xš‡2?%:
sýg:?(™¼xš‡2?ïC|«ï~ö?¨¢â#÷®?—j~ …K?¨¢â#÷®?ïX.½$?']¤8œä?"ð([z?']¤8œä?ïõW»±O!?Læ^íçø?UPˆp¿³?Læ^íçøAGN3FGL J0850.2-1214@mÕ¥€Ãÿ@3‡aÿÏX˜À8#¢á@øÀ;'\Ôm*?öÄxWª‹Ú@C™DµÃ@R‹Ö7"§¿Þ+¹½âŠ_¿âÀûˆLV¿ä¹2X9Io¿èܟEðAGNfsrq@'~ÊW§†ÂLogParabolaPMN J0850-1213?ï÷càéÔ?PŠ»ÈR¨?Q8>ŸÊ΁?PŠ»ÈR¨?ïÎóò;ØZ?ŒÖeNyºË?x†ÿ w?ŒÖeNyºË?ï"Ìæ֖Ù?†
MJª€ï?ŠÌÆT©È?†
MJª€ï?ïý
?§"`?$@rÆÈ$_?7®AwHÄ?$@rÆÈ$_?ïÞÒø/?q¨ècÄ/?p–ð에{?q¨ècÄ/?îö=Î}?³Ýñ³6V? œ('-?³Ýñ³6V?îs­Æėl? îÙÕÞi8?¨Å#'þ»I? îÙÕÞi8?ïüS"{>)?8øQ²w5!?=cÛ¡B+?8øQ²w5!AGN3FGL J0850.2+3500@g‹gk*@CBî¤ûÍÀ:—6JÿÀ;÷3I¨Q¿Ñ›>ÎË]@ÁläÚµ™?þ¼òÿçVf¿ë>rH"¿Å¯c)ü˜¿Ï",¹úì¿äÏ$;&OSAGNbll@¨¢múCþ]PowerLawRX J0850.5+3455?ïþðÇü?$àÁj¨É? þóŸÙY?$àÁj¨É?ïÚ\£«&›?'ž1 6ëÊ?rÑ®2«Âr?'ž1 6ëÊ?ï⿋×Ë??e"ÛÀßD{?m@t6Q?e"ÛÀßD{?ïñuAåA}?F(e—¡ä?]|Eû&Ç?F(e—¡ä?ïügôÓH‰?<1_vw{J?<ÀYŠb?<1_vw{J?ïFK}Ï0!?˜ÎõqѦ?—6Lù3Ü?˜ÎõqѦ?ïÔ&«Ãñ:?uS7½`
&?uìª?£?uS7½`
&?ïfY]¿MÞ?ˆª¥©f?"4ÔM=®3?ˆª¥©fAGN3FGL J0851.8+5531@d>—?·¥ô@Cx†¿¢AßÀ:2)ösDÀ<¢nTqq¿ý<ÒvYùq@ó!i1Fõ@½3@IFE¿ç«—SKà¿àædçn—¿ßI°¹¬ð ¿ìéìPS](AGNbll@-<j~ùÛPowerLawSDSS J085135.93+552834.5?ïà=/?tÜ º(:?oÿ€¾ØH¦?tÜ º(:?ïå·â&r¨?x-Å«[f?jHݬà?x-Å«[f?îæðA'J?"7ÿb۞?¡ûîÖëg?"7ÿb۞?ïÿïFýÈ÷>Ù1¶Akq>à¸Ùª=<>Ù1¶Akq?ïãOÊ\sã?mR
cÌËN?l°5—-"ü?mR
cÌËN?ï?à2ZE?¯ÈvúþÑf?˜ûl…U?¯ÈvúþÑf?î$!Éî?£§ë.¿?­½ã^‹Zú?£§ë.¿?ïþkF䯱?,­âá+ƒ?)K'ìÞ?,­âá+ƒAGN3FGL J0852.6-5756@q5X ÕúÀ!ù€	$ÂÀ8иϿÆTÀ;Vóâ»K›?é¹òïÔ6@·÷¨˜@9ùŸ"®ž¿â3ªÏ¡éI¿æaBq>²¿äòŸ¿Îa¢¿æ*í;¾XAGNbcu@‰ÅˆÞ*Ã"PowerLawPMN J0852-5755?ïþÏ¡=|ã?'§7Za"?#ê¸õ(ï?'§7Za"?ï‰7‹ sØ? @Nofϟ?²Iý? @Nofϟ?ïÚ@˜¡w	?oj1jdÜ{?rß³š¦ÓÍ?oj1jdÜ{?ïÙJ…EŠà?QoŠœd›Ô?sZ½dÉ´?QoŠœd›Ô?ïû`Mj
‡?Ew\Aš5?B~Êf¡Ì_?Ew\Aš5?ìì0sv€v?Á_Œ³Æ/?¸ž|fÊM?Á_Œ³Æ/?ïMÒÅ?'$õÑÕŒ?–]i+ãj?'$õÑÕŒ?ïH#…ɶ ?‰Ùʘ_?–ûM¨cé?‰Ùʘ_AGN3FGL J0852.7-4631e@p§Ü_|gZ¿óº_y5À6£Æðù²À9Ú¯ÿ6¬d?߬÷šU×"@",dŒòl?ÿ6í棿ÝßtDJ‡¹¿äjñER¨¿â²à6áé¿Éx/fŸò#OTHERSNR@«°‹ûµtPowerLawVela Jr?îÞP'EâZ?¸ŸÉD¾1:?¢÷Ø2>h?¸ŸÉD¾1:?ï`$n…í?«îTçû?"ûr*(˜\?«îTçû?晪JŽ;?´ñ´wÔ=~?ÒÌ«jã‰ä?´ñ´wÔ=~?ïéùÖLÂ?TìP½ÞA?fù÷N?TìP½ÞA?ï7éæ¹?¡7j­ s¹?™Ã,N¸V?¡7j­ s¹?뛧™ó—Î?Çð«†"Æ?Á'a˜1 È?Çð«†"Æ?ëÍrFü?¯Skás¥?ÀÊ6çÀœ?¯Skás¥?ïk¡ÒUÖT?ˆ´‰L(ÿQ?'‹ÅµE5ƒ?ˆ´‰L(ÿQAGN3FGL J0853.0-3654@p2*Ÿ{Zê@ÑÍÀ<ƅÀ9IÏQâJãÀ;C*3<m¿-|ð(@çúU:n@yÀšºV¿Þ[âòí¸¿Þ´<	œX¿ß…±.Ov¿âe `jAGNbcu@¥	‹ûµtPowerLawNVSS J085310-365820?ïûc'æ;?>t–,º?Cžqàûz?>t–,º?ï±Ói@'É?Ÿ¹"ξ?ƒ‹%¦ðQ²?Ÿ¹"ξ?ïÍÕc§ÍÂ?uK%?yNúÖÛ?uK%?ïåËÁˆ3?PµçG?j4>í™Õ?PµçG?ïå¦ù\*?fÚˆd?jYc<×t?fÚˆd?íjÕ¿mF]?¿ìKÿC'Ù?´©R•Í?¿ìKÿC'Ù?ï"È‹8q¥?‹è`暊M?ŽÍÝC¢•?‹è`暊M?îõ),Ÿb?ŒžJµ.@G? ­m6Yà?ŒžJµ.@GAGN3FGL J0854.2+4408@fÀ‡D,@D	e4Ù&À:ô°ÿèÀ<Ü»W?ߚÖÌf0È@íÀÓg?ü󚜲ÿ¿ïþ˜˜s÷?ïí–@ž«§¿³'÷þm¿æô·µ8†"AGNbll@°¯G®{PowerLawB3 0850+443?ïýž"[D?4cüú>N­?3</œò?4cüú>N­?ﶗIïH‰?Ž§#&XT?'Z-'<a³?Ž§#&XT?ï¹îª±Þ¤?ÚMt˜$o?"UM?ÚMt˜$o?ïY¢LŠa?…Vdãð`?Ë»–Ø?…Vdãð`?ïäæFp|À?sÛ{½ÝÑ?k¹ŒÃ@?sÛ{½ÝÑ?íôªmøg?µ'šiõ¨h?°Z«•ÚD?µ'šiõ¨h?ïP?/ë«	?'–x­®A?•øùó˜á?'–x­®A?ëòÀsšy?´d…ܨ€ö?À7°þ1–?´d…ܨ€öAGN3FGL J0854.8+2006@iÙÔ?u'@Aèä€G¸üÀ7'tvÊbÀ:ÕaèRdQ?óÙq±s*@ÜÉ܂wi@žåE¿|Ø¿Þ¤Sʋ·¿äL
2n¬¿â.V#Åyi¿å
•Þ½ÕAGNBLL@†\=îxLogParabolaOJ 287?ïÿ0_T'?úY¬%ƒ¹?ìQ;\`.?úY¬%ƒ¹?ïàSO»Ýš?|³€˜'BÃ?o¬°HAî#?|³€˜'BÃ?ïÅ©Ď÷?€üºüä?}+v¸"Ž?€üºüä?ïÿ#J8A?	‹·"pÊ¥?–¿½
¹)?	‹·"pÊ¥?ïþä%ü5h? ÅøûøÏ?!½¡Þò? ÅøûøÏ?ïC…cæ?«aÄJ…$ç?—_÷ÿG?«aÄJ…$ç?ïº`¨P/‡?‡Ž‹-!©?gÕáý@G?‡Ž‹-!©?ïÿîÉp?á©óïÔv?Â9ý"fª?á©óïÔvAGN3FGL J0855.2-0718@ma¿ "_ž@7SÎß̃ÒÀ:º$TÀ;ÅÔî~:?èäÄÛfÃ@ Ì@Šà@…#`,e¿áèyÛ°ŒÈ¿çq÷¦a {¿ë&þ¿ïñۙ2/lAGNbcu@ƒú5?|í'PowerLawPKS 0852-07?ïìêŠ*™d?`‰b6ýR\?cvãf?`‰b6ýR\?ì	¨vðæ÷?¸'Õ°®ÛŒ?¿²¼HxÈF?¸'Õ°®ÛŒ?ï7[3WpT?…»9ýQÏÖ?™™š9_o?…»9ýQÏÖ?èÀmÿ7? Úk×û@?Ìÿ†H#÷? Úk×û@?ïÈÛê)²Š?xÐ+À÷?{'"û?xÐ+À÷?ÖѼګ ™?Йf›%Ç?ä—!'ªo³?Йf›%Ç?îD˜Žß#?ËžÑN?«¶w&Ð?ËžÑN?ĶeÜ[i?£ªDHśÊ?êÒ{æˆé&?£ªDHśÊMIXED3FGL J0856.5+2057@i¿¥_5½@B?l?Ä;.À9²E¯6¹ÐÀ;!¸·l¿ë;¯P @À7·Qex@|Ì¿`Ó¿çéO?Ù¿ãdÞKy¿âkt}UkA¿Ü-I~AGNbll@ §ì¥zxlPowerLawTXS 0853+211?ïÿ6&,ºs?Je'Í–?;:ð'Q×?Je'Í–?ïÝþž‰¡?ƒˆá=©?q°£"8Í?ƒˆá=©?ïëœ9mE9?eº=ø	ñ®?dcÆl?'5?eº=ø	ñ®?ïÿF³(òú?ç'™½	^?)¡³6y>?ç'™½	^?ïþšgtÙF?"sÔ&M{?&Y†Ã£å??"sÔ&M{?ï< ";ÛÆ?«ÎTIHí[?˜kï{ô#E?«ÎTIHí[?ïÒh,0¬è?zó>	Õ³¨?vËéßj{Ï?zó>	Õ³¨?ïóa>3li?R•
åËo)?Y=ƒ}ªN?R•
åËo)AGN3FGL J0856.7-1105@mÔ¾ Ìÿ"@5}c`!¨ÇÀ8Ku€µÀ;ºßd?ð5`ç÷J¥@Á©Æ˜@gUê¿Úfñ£N'¿àúÑ©Á*¿à>'D´Ý9¿äYìý¼%AGNbll@"œ¼¹#¢œPowerLawPMN J0856-1105?ïÿõX²?
€%Füb?Qµðˆ¥?
€%Füb?ïp>iб¼?"åґ¹¤?'ø2ÉYdp?"åґ¹¤?ï׋‹J1¹?tU´Oÿ~?t::tT??tU´Oÿ~?îPp¤äü?'n­øT?ªøÿ†—;?'n­øT?ïÿ¸P'¾?!br7	Œ«?èüäݱÂ?!br7	Œ«?ìdœ?o?À¨Ä¯ÇÙH?¿ßÜÛ‰?À¨Ä¯ÇÙH?ïÀd›Rh?"¼¡/á?ÍñÑó4?"¼¡/á?çûá ŽÂ?­7ó¤az˜?Ð<¿Îâ|?­7ó¤az˜AGN3FGL J0858.1-1951@nÊ?þó†@0‹hß½jYÀ9N^¢LƂÀ;€ûŒ3€?æÙq/‡@Äf1¸3ä@³¢ ~e6¿å¼áÀ­bW¿ã8؊ßÜ8¿ê],¿.\<¿átùg=.'AGNbcu@"¼‡ü¹#£PowerLawPKS 0855-19?ïÿHpÃGÏ?_u}¡?ñï+'ò?_u}¡?ïÎÞL¦÷¦?…£4%‹$Ã?xÙŒ7Ù#?…£4%‹$Ã?ïËØìYŸ?qIÊÉoN²?z~›<…?qIÊÉoN²?ïì;[º²?EJ[¡J©?cĤi<=Î?EJ[¡J©?ïý¾{jo?6ô~u?2%UA_?6ô~u?ï`ÒJ1Ÿ?ª5äø`B?Ÿ"å±'b,?ª5äø`B?ïKïO-º£?ŽÄ3øµF?–'Ý˜?ŽÄ3øµF?ïz¨ìYV?":ôú?ªâtÝU9?":ôúAGN3FGL J0858.1-3130@oô/ ê[S@"p@Õ³PÀ:Z­ã×À;Jaοõ5D°^,@â?j¤
¼?û³˜Þ³ª¿â8[¹íª›¿ãyù»Ã:'¿ÝÌ̀i?¤½Üfj:AGNbcu@¿¾–âëCPowerLaw1RXS J085802.6-313043?ïþúrˆ™Ó?"ÏÜO­? XÖ!‰Žq?"ÏÜO­?ïÆëÄ+5?‡ôΣ°?|ŠÛ÷!á?‡ôΣ°?ïßI{Ú?nk÷Ïj?pqÛ>Éw)?nk÷Ïj?ïÿôým~‰>Ó=˜;ž…G>Öžiþ¯>Ó=˜;ž…G?ïþ,a˜?*D­<Hø'?-9ð~ˆ_m?*D­<Hø'?îϤŽüv?´u|m³Ñ?£¾'ĵž?´u|m³Ñ?ïÂ4…?t0døµ?~õõÇ	AÝ?t0døµ?ïÿ ¤ÒO?!,ÇUl?ë{+³Ñ?!,ÇUlAGN3FGL J0859.1+6219@c%°_®¼A@C?'à°«À:RV	!òÀ<wJº8v¿íÒ=؆G@àc¶Þ£å@u‡_…K¯¿âÛ]ë‡fÖ¿ìąz¶?¿Æ>ôff3¿êÔeè´ÒAGNbll@‹ðÉAÈ!lPowerLaw1RXS J085930.5+621737?ïûQ'S¬Ð?V"‡|Ü­"?B¹õ·µìÇ?V"‡|Ü­"?ïÛLló¦ß?‡9æ»aÈ?rYɂ¼ô˜?‡9æ»aÈ?ï yDª?'˜BDÎ3?‡á®íO	?'˜BDÎ3?ïþW€¼ËD?P­[9È?*‡ö'ÕD	?P­[9È?ïýWð	›h?8¶B[Ã?5@Ztžð?8¶B[Ã?ï+ðd½«?­Eãü°0?šóo)×µ?­Eãü°0?ï™Íž%fä?‡÷,ÄD˜)?‰Œ˜s6ªø?‡÷,ÄD˜)?ïì8‹Èܹ?aÛÄÀŒ?cÇtFŽÃ?aÛÄÀŒAGN3FGL J0902.4+2050@iÕ³ S\ž@Báj@ºˆÀ9Ñy÷ÜÀ;w˜³ÀŒM?ãjñÎÂxé@~<)Ñàˆ@Б_äA3¿Ô	V'
¿àDÚõ{äõ¿â
C	÷Æ¿áhCÄ×OAGNbll@—¶Ü¬1'PowerLawNVSS J090226+205045?ïÿªJè\?ð>ä¥Øä?~é(#z=?ð>ä¥Øä?ïØÇ뢷?÷ݪg2™?sœ
$U¦¤?÷ݪg2™?ïÙ÷_Èg?uƒ-Áä!a?sP;ÕO?uƒ-Áä!a?ïÛÃíw‰œ?Q=ÖW>›?r	C‹F ?Q=ÖW>›?ïÿ8'°ýl?ޏÃÝv?ïªvK¯A?ޏÃÝv?ï&¢_L'?¨V훦–?›+´%-?¨V훦–?ïÕèn¶8ƒ?B€ÌLÙ?uÈ¥"ªo?B€ÌLÙ?ï%<_¬¸Û?†¹Š¸×?›Xt
؀–?†¹Š¸×AGN3FGL J0903.1+4649@e¢£¿ø¨ô@DÊ:?–îÄÀ:ªÐ"£À;þ>Ëí©¼ÀÈô>«·S@b{üû"@ꀿƒ
;¿å̪*éì ¿ê§B5sn&¿×ÏE%V¯B¿ïú´ù¾¿»AGNfsrq@€ÊêJŒPowerLawS4 0859+47?ïü7åä9À?<ó7×^L?>@ÑÙûǘ?<ó7×^L?ïäñӆ>7?|NÐÙ²õ?k,¢ýæ?|NÐÙ²õ?ïvó-?~Í%
ôN?'?a˜5d?~Í%
ôN?ïÿÿ«,¥6>•U›¶4Û­>…'§=¤ŒY>•U›¶4Û­?ïýƒ©¨?7Ðá2l8?7»ãÃ^?7Ðá2l8?ïImüÕ¤?ª±'LÑ5?–Ò@`4¡‡?ª±'LÑ5?ïf<€AŒp?')
úÕª´?"8oþ­©ù?')
úÕª´?ïÿêÓÀSd>ôèµvÌ>å,+x">ôèµvÌAGN3FGL J0904.3+4240@fSÔà—"ì@Dña_–hÀ9øE~RÀ;åٚ:©I?و]·k;¸@j3óL"W@ο¿É?¿Ý2`Ov
¿ë¬Bn~¿áàʐÀW¿ãÖ–íAGNbcu@‰yýŸÓo~PowerLawS4 0900+42?ïÿ²s–`æ?Ãa>V›œ?c7³.Ô?Ãa>V›œ?ïÔù×û\¶?ƒÕåFÈ?uƒ Ž4õ?ƒÕåFÈ?ïâÊYC×à?^ÖýJÁ‹Ð?m5¦›+àD?^ÖýJÁ‹Ð?ïêõ_p±?g3U}mš?ˆ…BµâC?g3U}mš?ïÿƒ×¡£:? ¦JG#U?
Í~c}? ¦JG#U?îs³¦©E?±N
›¶#?¨Äş	"´?±N
›¶#?ï—v<$üí?‡:ÓõçÌx?Š"pöÀÄ´?‡:ÓõçÌx?ìVՊòþ?¥Wº:Ê?½IS¨k?¥Wº:ÊAGN3FGL J0904.8-5734@qA¬à2ÛÀ! ßÞøHÀ8W,ˆõ¨À;.Ãø贊ÀBjØf@Tꙇ¸@›ÀSu¿æë!{r3œ¿â<>.äÄæ¿ãëË'(Ù¿ÞÿM»8êAGNbcu@ûŸQìPowerLawPKS 0903-57?ïÿm#w†þ?ŒÝ°©?[–¿Q½Ä?ŒÝ°©?ï°îº³D»?"yüòä¡p?ƒÄQQw&?"yüòä¡p?ïÒy·K?|ÃÅ{Ië?vÃ`¦:"?|ÃÅ{Ië?ïÿþЪýÅ>§¬H›äN´>¢òÐöt'>§¬H›äN´?ïýäü]Lü?.ÃßGwÖ?0Øn§™n?.ÃßGwÖ?îÇÕ0|?¹ê¤ñ]ó?¯ã'ªkƒD?¹ê¤ñ]ó?ïœàKO½?‡µÁï<œ?ˆÇí<tÍ?‡µÁï<œ?ïÿâo»ª>ò<'Ð@¶M>í'êÇM>ò<'Ð@¶MAGN3FGL J0904.8-3516@p7߬£b@R ß´+À8¤ÌHBŽñÀ;NÞ̀Pó?çB4E,@Ž )֓@4TçÑá¿ä]ÅÀ¾÷w¿èQKòœÀ¿è	YQnÌU¿ëÉvBÉˈAGNbcu@yg[ߏG0PowerLawNVSS J090442-351423?ïü=÷4?7'ïÅ
X;?>H
2UN?7╁
X;?廓ýa•?';‹¡}K'?…Ý9†Ò°?';‹¡}K'?ïƒ×á&÷?†[ÂèU;?
vˆ6_?†[ÂèU;?ïÎÅlJî?Yôh@û±?xIº¦µ?Yôh@û±?ïúCéõã®?FÜJAžî?FðXuh‰?FÜJAžî?í¥íûE±?¾$o‹~"ñ?²Ð%d"?¾$o‹~"ñ?ï:š%Ç:?'ãªüñÂ?˜¬»aæ¼?'ãªüñÂ?îèyšÞ¤?‹ý´Ùãw
?¡xo	ã¹?‹ý´Ùãw
AGN3FGL J0904.9+2739@hÎrà\̊@DE À:W%ô†O:À;å)äÕØ¿øĦf%Ï@
);}"@DßX¿¿èfŸ=ò2¿êqȜçVç¿à4>&}Ô¿æØÿsú3ôAGNfsrq@€êzáG®PowerLawGB6 J0905+2748A?ïÿŽ,Aì"?Ôôd:¾?tô¯æ?Ôôd:¾?ïáù;{E?€üSlv?nïÁÅ
ú?€üSlv?ïÛÔkôè?cuxbŸTí?rÉùÝHê?cuxbŸTí?ïÿ¨i«V>û "ÊuO?廀Á¹¬>û "ÊuO?ïÿ[¿2IB?¾Éé§Å?ˆÇ.Îú?¾Éé§Å?ï[‡Yiís?š2¢ÍF…¦?"ÒÂQ–?š2¢ÍF…¦?>ùÄ?"ñ	a
ƒ}?‰ZpHnW?"ñ	a
ƒ}?ïö\W½}?R¼Íê›Í ?SGR@;ôÁ?R¼Íê›Í AGN3FGL J0905.5+1358@jàÓ`Ð$p@AúQßƤ•À9öŸ..À;B̺XV¿Ç½úÏñ@"gtƒ_›?ýknî1÷?Á‹á.Gà¿Ü¼pá6Æ¿Ýĺ]€¿Ôš:YÔBôAGNbll@¥ß¾vÈ´PowerLawMG1 J090534+1358?ïûêeJBÕ?7Á7:À½Þ?@Viùgtê?7Á7:À½Þ?ïà	ƒÈˆ+?t™s^êl«?oö|YÓí?t™s^êl«?ïÇVGN7	?y1E'ôHn?|TÜ9÷ÿs?y1E'ôHn?ïù Lsœ?5|)ò£›
?K~Íàž3%?5|)ò£›
?ïóO'k¢?W
á>[t?Y`úï'j?W
á>[t?ï>{¼A—Ù?§×Ùâˆ@™?˜0ˆ€d
ä?§×Ùâˆ@™?™à!¤?ˆvõÞF¥^?‡Yz9&ô?ˆvõÞF¥^?ï¾£eÊ?t%YYü3a?€W&˜s;z?t%YYü3aAGN3FGL J0906.3-0906@mËýàÖo
@8• ŽÀ9l'^;õzÀ;ƒ0"'¿ÀõTͯR@-Ñ4§@, šTU¿Öø±*"¿âû/–pšG¿ßi²·#¿ß:*šÐbAGNbll@žì<žìÀPowerLawPMN J0906-0905?ïýéQŠ-¸?)Ì{­n7i?0µss2—à?)Ì{­n7i?ïڎõâÖá?©"¨À`Õ?r¸…!"s¢?©"¨À`Õ?ïâ¾±V#Î?fѕ0õ)?mAN =Iý?fѕ0õ)?ï÷w¶…Û?87E2EÝ&?Qü…5Ú9?87E2EÝ&?ïùÄ¿É??G3$ܵg?IÀì!Ú?G3$ܵg?îþwݺ¹X?±«cÌ|F­? '#xƒ‰?±«cÌ|F­?ïºÆ˜ˆÖ?'«~A¦ó?NYÐd¯?'«~A¦ó?理c	|?w€üÑ1?†ç1®Ìý?w€üÑ1AGN3FGL J0908.4-4916@pä˜à†8¿ñ(Hÿ"_{À8r.ÎI¤À:VZ°O¾"?ä³m»@ÚÍÉwê@"]60¿¿é'íø…Q¿ç׋—£J¿é÷a¿Þõ^®XÛPSRPSR@"¿Œ~($PowerLawPSR J0908-4913?ïn#ÿ0Ä?œÖ
Ù«"?';€""íw?œÖ
Ù«"?ïGp,ù?·ôØR¾ž?·ñçZå?·ôØR¾ž?êˆû©?°¯Þf"?Çï‰ß¬Z?°¯Þf"?ïE¾¥$?v-D']J?—H?$|7é?v-D']J?èJR+u?É¿'c­_°?ÏþÖ·S¶-?É¿'c­_°?æÙÏǨö"?ÌC%R¹¥?ÒL`p®ø?ÌC%R¹¥?äxôÝPíG?Àlµ[¨-—?×E^%r?Àlµ[¨-—?é
Ò¤/A?µ¤ÐòZ×»?ËÈ·ÁoBû?µ¤ÐòZ×»AGN3FGL J0909.0+2310@iŽŸ¾vÉ@Cö?µ!µÀ9š@€MÀ;`¹4i"¿ü
½áÍe@*ÏÝMy?û`àÀt¥¿å¥<Ê¿ä9÷;D"¿ª¹;9UÐÜ¿Ônô'¥AGNbll@¶JKŸU›=PowerLawRX J0908.9+2311?ïÿ‰Ø±\"?¸=ç­?
‰ÏOI+£?¸=ç­?ï⡯ù¿?X"nr?mô^\dÙk?X"nr?ïñbE??e\òVm?];ە=ò…?e\òVm?ïÿþظ"Z>ŸÌ%ôÒ>¢u€Ht›…>ŸÌ%ôÒ?ïÿ«Æ0À+?ڌÀÖU?qš?ڌÀÖU?ïhK+ޑW?¢
œºb?'öš‡q)?¢
œºb?ï컑Þ[¸?nï‡ù›Ö?cDn$è/?nï‡ù›Ö?ïÿõMõVY>ÛܟÕC>Õdnn	Çi>ÛܟÕCAGN3FGL J0909.1+0121@lžj_"ÊÕ@>íÏ ¼£ŠÀ7Ø:ø‰À:Ì;ëh™?üj%
%É@uÔÔÙ
É@AÔÜ:Óæ¿ã'xµ•Åò¿æ–èžÜÆâ¿åFi÷óö¿î5 é¼iAGNfsrq@¼—$tTLogParabolaPKS 0906+01?yïÛ?›:©ìovÓ?‰›!vJÉ£?›:©ìovÓ?ïƋçC4w?…Ö¦ò­?|ºOG|ž?…Ö¦ò­?ì§'"?¨¬"ÿ¦—C?ºÇ¦ÃßÏo?¨¬"ÿ¦—C?ïuð½ËZº?uxƒh
›†?'AèAm>º?uxƒh
›†?ï‹?›˜Äª?Œvøú‰;?0?Œvøú‰;?îÀ¦0ßN?¹pÀÜyt'?£õœò-?¹pÀÜyt'?í<=œÝ_±?¤ßjüP²›?¶'õù?¤ßjüP²›?îôü,ìr?"êrÖàlª? ³Ä:ƒá?"êrÖàlªAGN3FGL J0909.6+0157@l_ 'á@?W°?ÎL)À8û̈Ú.µÀ:îÁðи?ÙÅc@0
¤@wœÄœR@T/ŸªÕ¬¿×ÀÁ`¤Ó¿è¡ ¹*zõ¿ãOÿô¹È0¿ïþÎSNusAGNbll@'&€IPowerLawPKS 0907+022?ïmÚ¶Î?˜§¶è´à?Ÿ'MÝÉîM?˜§¶è´à?ïÊÁø»ñ'?"ÎT½»?zŸ²…W|?"ÎT½»?íQOomºÝ?¡øöâ¥9?µu""')?¡øöâ¥9?ïuŸÓ´6m?p}žû$i?'L"QÈo?p}žû$i?ïÎÏÜÿ?…òOԃÄS?x˜~‹Q$†?…òOԃÄS?î"&¤?Ì?°‹Ä/I ?¦½•¼?¿?°‹Ä/I ?ì½ôªâA?¨À¤Är?º Z¨íõ?¨À¤Är?ì
æÛÁ²<?¤Ò§ì¾eÉ?¿¨É!òn?¤Ò§ì¾eÉAGN3FGL J0909.8-0229@m9pޏ@=ìð{(À8Æ,p¡RËÀ;ƒ†.'ÊJ?øA¡^›@ŽßZn
 @"•úR¿ׯ"[ê¿å9Z£æa¿ãÏý‹RüI¿î'´m–—˜AGNfsrq@€è1A [ÀLogParabolaPKS 0907-023?ï‹d¸™í…?´'Q'Œ¨?&ÑçC«?´'Q'Œ¨?퇓¿‡aU?²ŒäXál?³Ãb|ÃT?²ŒäXál?馥(C)?¯'ˁ01Å?Éek^ó«^?¯'ˁ01Å?êcþ9¬I?›)™Š?ÆpNۅ?›)™Š?îbíQô?¨ÝÕ#Á?©Ñ*ï0¾©?¨ÝÕ#Á?æKZFûð"?Ê<U¯®‡?ÓiKr÷?Ê<U¯®‡?èz­	?µ×³Ϗ?Ï«»êKÛ?µ×³Ϗ?ßl¤¹2f/?µ¯ïx´¡Ò?àI­£fÌé?µ¯ïx´¡ÒMIXED3FGL J0910.5+3329@gã×@Än@E:íàBËWÀ9!þW‰TÀ;T4£u»n¿×,If»4@oÀ£ÉžD?ÿ¿/ •A?ßàÜn€fB¿åwuÂÏÈÖ¿Ý1i¿Øτ!¸6"AGNbll@§jîæ1ø¡PowerLawTon 1015?ïÿµ¨v‰Ó>ýuqØB3I?•Þ:
&>ýuqØB3I?ïÜä jG‹?ƒðbø΀}?qï½Êo?ƒðbø΀}?ïå-—Îú`?mÝÜùB‡?jÒh=d81?mÝÜùB‡?ïþwâî*?;ØÝÂx"?(Hg$`?;ØÝÂx"?ïÿ±jÒÃ?Äaî$h¦?œ%» ?Äaî$h¦?ïW
u'Ž?¦ŠñzË?•^3Ü9?¦ŠñzË?ïàÎr¥u+?|™¡4l;?o1]J"Æ?|™¡4l;?ïôIqÊu?P#ó!ZóÙ?Wm¾m•°?P#ó!ZóÙAGN3FGL J0910.7+3858@fö@ÈG,@EÈ?ŸR@À:á6U&£À<]\Òhî?Á8Tú3@Vöï‹Ã?þè`§	Å¿àò
·'$?²'Ÿ¾2…¿áø@{+¿ÌhØÞ VDAGNbll@¯øQë…PowerLawFBQS J091052.0+390202?ïýâÃH'?:UFHý?0éãÞUfT?:UFHý?ïÝ>ë*äc?ƒ`åkÔ¸G?q`ŠŠ*6p?ƒ`åkÔ¸G?﹩æ)%y?~qOŅpÆ?•†wno¡?~qOŅpÆ?ïÞOçâ[?YtÃ9è¼g?pØwvÁ>Ú?YtÃ9è¼g?ïá¯ìÛú¬?vL">Ô+²?nPÔ-?vL">Ô+²?îèÏT
?«½íEo<?¡sŽŠ¿.?«½íEo<?ïUkèd
Ÿ?ý¨Zÿ4f?•R'öîH?ý¨Zÿ4f?î#±GW¤Ï?£íþ®mÒq?­ÄëŒ=?£íþ®mÒqAGN3FGL J0910.9+2248@i¢Ÿ<pÊ@DƒڐÛÀ9'4èÀ;—;-C/?â=€á^K²@ŠT‰š"@É eϿ׋ͮt2¿ãtÂ6ñ®®¿çuᚌž¿ë_[XÑAGNfsrq@‹é8Që…PowerLawTXS 0907+230?ïôq]%ê?VfâÖ)ª?WEñüu?VfâÖ)ª?ïÞå¡@=?}}˜Bɾ?pö
 A™s?}}˜Bɾ?îªÜQq"?—6Ó؃?¥R:ë{s?—6Ó؃?ïðÒúZÇ?A'e.¿?_òZy=ñ?A'e.¿?ïìaŠ‰†Q?gI¢`gžË?cžužU&¶?gI¢`gžË?ï/s5µL0?©ªyŽ&í×?š™Gž«û?©ªyŽ&í×?í"têΛ?¢ä/ǜJõ?³dX¯™‹,?¢ä/ǜJõ?ï§9qTšÑ?u
w7Ñ÷?†1££úÚ?u
w7Ñ÷AGN3FGL J0911.8+3351@gÕ¦°)(@Ec—tüÀ:7‹dL°³À;™¤µVŽ'¿Ý/¬	Lž®@
bmÔï°ý@Ììš"ì¿î7á…ä¿«ÈMÙt¿à
_¿O®¿×ÏI_«cAGNbll@ª›&$Ý/PowerLawMG2 J091151+3349?ïÿÝ5¥©?ñ {"¬v?DS)0'Ë?ñ {"¬v?ïڍðn«?…Qr´3–?r¹§úêq?…Qr´3–?ï瘲‹Ov?W÷µ–•Ò<?hgM›,)s?W÷µ–•Ò<?ïü5ó#p?+'&\£Ø?>Pe$ÿ?+'&\£Ø?ïþ2.•-"?%G®~ە?,ÝçÇÈÏ?%G®~ە?ï=uFܐî?©\'Ptâ€?˜QW$mâJ?©\'Ptâ€?ïÞÆù	|è?q&
'?pœƒtbT=?q&
'?ïÊRúMäd?rïße9ð?zւލ-Á?rïße9ðAGN3FGL J0912.2+4126@fŠ¿ðEx@E«³ß•ý-À:_›q
.À;ÛßÞèX¿ÍÐU5¼@
:MXÎM@Ч ¿ê™'Îr‹°¿æ	7ÖÓXO¿èÕ5Ú"©?–sáÏwQAGNfsrq@"ß—>«6zPowerLawB3 0908+416B?ïÿëç*'F>âi¡:$bb>äΧN>âi¡:$bb?ïåj
	ï?tkÈÅä?j•ö-ð·?tkÈÅä?ïä藮‡è?ZŽKB­©?kh-¼'ð?ZŽKB­©?ïÿ²nÁm>ófõZÀM(?dAsÓt>ófõZÀM(?ïÿބQ«;>ò	 «/=w>ð½ÀíÂ>ò	 «/=w?ï6šÖõ4?ª¬DÙ-@F?™.ªHÇ?ª¬DÙ-@F?ïÊÏþÊ9¹?wÞ9èO3?z˜¡Â[O?wÞ9èO3?ïûÞÞ¥ÅÕ?=&x>®Œ»?@"…øñã(?=&x>®Œ»AGN3FGL J0912.2-6452@q£˜¿pÀ&~wÁ½oÀ:
ÑÒÆÀ;­QU])§?Ú±¿ë³@Óá:(@tߥíe¿ädùŸÕE¿êÐKÝN¿Ü|í¼[u¿êÏœ'r^OTHERglc@TûµsëPowerLawNGC 2808?ïî\r$hH?tOWöõâ?a£Ž
Rgú?tOWöõâ?¢ Ã?˜^¹†ºgò?W[>Ô¢?˜^¹†ºgò?ï"Öü?ƒ àÒ¤*?‹:þÃ9Ý?ƒ àÒ¤*?ïf‰YZC?qÛ%6˜î?".ÔÖeå©?qÛ%6˜î?ïÉú–Dá˜?—Ç"w'?{´ÈñŒO?—Ç"w'?ê`ü!ן?Ä5Ué&ÛÈ?Ǿ|x¡…?Ä5Ué&ÛÈ?îÄDzÙ:?š-,dá Ú?£»¸OØ©|?š-,dá Ú?ëSDNI~?ª¥ß'	M?²ïšÆÚ?ª¥ß'	MAGN3FGL J0912.4+2800@hÐ_ôö@DðãõhÍÀ:sḻôÚÀ;¥Á*[J?êpl÷м@¼™£Õˆ?ø¤¨¡s3?ïýð'
g¿å#º'ê»Ü¿ã!W:é?Übö¨œAGNbll@Á–²-VPowerLaw1RXS J091211.9+275955?ïý=(2+Õ?:÷'¥Úï?6¿7×EH?:÷'¥Úï?ï܁{É;?€‹ïd·Ç¥?q¿B'xt?€‹ïd·Ç¥?ï—e¥~Ý´?‰\Q%Ð?Š&–‡?‰\Q%Ð?ïøO‹È9"?CE&…ßûc?NÁÐXõý·?CE&…ßûc?ïýbùۊ?BŠB¹§¤?7T潁&?BŠB¹§¤?ïK‰Òbt?¯™ó{u1Ô?žöŽÅ³±{?¯™ó{u1Ô?îúÈ¿æ¤(?˜m±W}Í? StYx?˜m±W}Í?ï¼`ª 
É?"v–ÎýÃT?€çՅÑÈ?"v–ÎýÃTAGN3FGL J0912.6-2757@oß<`Ÿ@+×n Ç‹DÀ9Ì(—ξÀ;—A<á?àÍåù;=@ƒhÄÍ$@"ö`o"¿êI:Û
$¿è–™*ø•í¿âV¬ƒ~¿Ýºfá¾ÿãAGNbcu@|üΤ¨ÁUPowerLawPMN J0912-2752?ïÿaÑpu?‰eӊ—¿?ÅÍ#NÜ?‰eӊ—¿?ï° ¯r?›Ø–?ƒ×Ô;ÐÁq?›Ø–?ïÝè²Ï6?s¸Î Þó›?q§¶­?s¸Î Þó›?ï°pÃØ?cÐî[DÀ?ƒãÏ?ê5ô?cÐî[DÀ?ïþ0øEv'?4ÅØ°CP«?,ðv¸‰?4ÅØ°CP«?ípr"»?ÀĬ¤°›`?·4|qÉ#©?ÀĬ¤°›`?ï‹!ÎKl?‰Çýë ?7˜"L]?‰Çýë ?íJN%ãûy? »+µqƒ©?µ­ŽÒ—ò8? »+µqƒ©AGN3FGL J0912.7+1556@j³|€"Þ@C)è°ºHÀ:dÛé*ÑÀ;><{±Q?ÛÐ?фË	@ïK"é!?õœkþÖµ.?䧸ò¿åÍY(¿ä¤ÖFE¶?æ«9åUAGNbll@ÐB†§ï²PowerLawSDSS J091230.61+155528.0?ïýb*A??Zíkðr-?7<î<¬'Ü??Zíkðr-?ïÝók•$?wdwÄnB?q~Õä»?wdwÄnB?îòMÀ°½U?›ÀŸlí>? Û#ó<\®?›ÀŸlí>?ïþù,§'ø?7uQg? m4±™‡Ô?7uQg?ïû
ÝÊ·?F¤šKÓG2?CȊïñã²?F¤šKÓG2?ï4ü§ìÿ®?®¨9Ô
é
?™`k¨<7?®¨9Ô
é
?ï 6¼Þä?•¬)i/ï\?›ù(k;w?•¬)i/ï\?ïòïÄ¿ý?c¼ËÃ"'?Z!üÞô%Ü?c¼ËÃ"'AGN3FGL J0912.9-2104@o3b¯È°@2zeÀN9IÀ9.66òÀ;Uv<?A¿×Í.E|z¿@«%󄜇?ÿä~ð ¿ã°ïÄsŒë¿àõíSļø¿Øõ@gô¿à¨&¿AGNbll@¦‰ŒIº^5PowerLawMRC 0910-208?ïý'φ÷'?(úøñ!L¢?3q…±‹Ïì?(úøñ!L¢?ïΉÁÆo¢?ô邂TB?x»;´ªû?ô邂TB?ïàšì;8?f³Û
96?obeT]o[?f³Û
96?ïúÚCOWy?0«¶ÏT¯>?D–ò¶ã?0«¶ÏT¯>?ïúý>Qê?>ÎâÛo˜??D8sŠ?>ÎâÛo˜??ï±~Æ7:?­»GƐ´?ž	Ð"®Æ?­»GƐ´?ï¿`~"£L?ƒ€º,蒏?€'ài@Ç*?ƒ€º,蒏?ïÈå>*)—?p–A'Góæ?{`ξhØ?p–A'GóæAGN3FGL J0915.0+5844@cŸVŸI@D¬à f§ÕÀ:®…à19À<%çbzH›¿íªf@%ßã@ÄÊ7J3@ڝ`˜¿ä%Š9eŽ¿Þ$Žq¿­L¿ë†k‰2e¥¿á錐òAGNbcu@‰È'RT`ªPowerLawSDSS J091608.57+584434.0?îÁóF£?ÊØí¹Îº°?®Cæí[ùÖ?ÊØí¹Îº°?ïÝ	p7?ˆ>¾'4Ñ?q{~7}Ä¡?ˆ>¾'4Ñ?îóô³›? d®èK³|?¦ðÀ´bK? d®èK³|?ïþ›îÕ؇?êe0±K?&Aa=ÅD?êe0±K?íÁkä:ã½?»¬·6@6"?±ô Þ(â?»¬·6@6"?ï-•Ðiíã?­Û¨‰€Ú¡?šMEïR§¥?­Û¨‰€Ú¡?ì*M°PÙü?²~wâ¦ã?¾­'}y0 ?²~wâ¦ã?ïÏþ4pA~?u†[^€ö?xå¶I ?u†[^€öAGN3FGL J0915.8+2933@h"žà*w£@Ewa_–hÀ8yœÇ]!À;ãÙq÷¿ÕF¾1­«@!B"ãÒ?þFA,ðú¿ÜÙ{ÞêþÞ¿Ûçª\-2¿Þ{å†#'y¿×+jš8âAGNbll@žp"uPowerLawTon 0396?ïüJ⸂¤?4ýÁûàm?=¨ëéӖn?4ýÁûàm?ïá èS¢%?†<ÙÈÞT?n_Â[[#?†<ÙÈÞT?ïËúeyß?wϊûœÈ?zÍ(Tz?wϊûœÈ?ïùð"7Ò?6¤¢Ü@aµ?H=ïi¶_Ü?6¤¢Ü@aµ?ïôÌñ	íê?TÃÏPGZ?Vfùâšï?TÃÏPGZ?ï,Hàïn?­O8MSŽÖ?švãÞ¢'[?­O8MSŽÖ?ﶡ‡y±r?†@'94<?'Wž ‹Á?†@'94<?ï´Å[¶¬q?y˜ÿÂwÇ'?'Ω5[¯?y˜ÿÂwÇ'AGN3FGL J0916.3+3857@fø{€©Þ‹@FÁ?À:qGZ1¤¾À;ð¨á59ž?ádû3ßÍÓ@ZáZxq@Ùhy?í[éTlê¿ã¾grJ~¿êÃa›³¿â~¨ÜŽAGNfsrq@'¿¢¶®}VPowerLawS4 0913+39?ïü¼[C%?CU1ì.?J?9ꅏ(L?CU1ì.?J?ïƈ›oˆ?Šn!Dn?|þ»›šÐN?Šn!Dn?ï[ø&Ì{?‹i
€m•Þ?"€ý׶ԡ?‹i
€m•Þ?ï]ºŽíÕA?{‡äÿR—?"H®'lÁÏ?{‡äÿR—?ïíŸÙà´?kù¾L Oh?b`&Bù;£?kù¾L Oh?î@T¼ÎZŸ?³D©÷¤€—?«ú´1bˆ?³D©÷¤€—?íH(qIŒ?¨‹L£"?µ¾¼u´ ?¨‹L£"?é¡!κkT?·ŸaÏGv?É{xÅR°?·ŸaÏGvAGN3FGL J0917.3-0344@mfˆ_Js@=äÀ_×,À:d7EçjÞÀ;²ȼœÔ¿ïµbXBiå@mó‹R"?ü7ë¿+N¿é8}RÈO¿×9[B"Dã¿ã–>¢@öÚ?¶ºÚM
AGNbcu@´Êäýó¶FPowerLawNVSS J091714-034315?ïÿ5Ø݄Þ?l~Ò?Dã¤N®x?l~Ò?ïÛUïÝì?†r;éu?rU­ê?†r;éu?ïç	B/5´?c½àa.b!?hö½—Ü~?c½àa.b!?ïÿ벍}Ï>ÚLQR×>äMAX	Ԅ>ÚLQR×?ïþD»4¸³?#£AwŠ™x?+´K1mœT?#£AwŠ™x?ï*¦ÍÜÈ?°`r·
»?š«&],˜õ?°`r·
»?ïÚzÓcrt?u^a|Í&(?r–Nö²?u^a|Í&(?ïþ%|Д?0¬4jCá?-®	Ëûu¶?0¬4jCáAGN3FGL J0920.9+4442@eö*?K@Fg€iFëÀ7ƒLŒ ŒÓÀ;6K\äÈ?üÏ͍'ùg@â$Læc@ž–Íar6¿àÎ"Ž[‰$¿å0ðÎ3Õ¿æôc6'§¿êUYyK£öAGNfsrq@v˜±zÌNùLogParabolaS4 0917+44?ïð̶§qt?h;bEj?^f'¨Þö?h;bEj?ïÜU‰|ô{?… —!¡?qÕ;N"Fv?… —!¡?îsðßóè?œM¬'Q?§(Àõp]u?œM¬'Q?ïý"°í&?".}hàtŸ?3g䕌?".}hàtŸ?ïÕ	ݬ÷x?w¡¡pXJ?u{>!ëç?w¡¡pXJ?ï8煾N?°PŽhÝð?8ãH6>?°PŽhÝð?íPœr}?§ëhg?·í{¹–"?§ëhg?ïý¾,~–¼?1²QËH™?2šFJk?1²QËH™AGN3FGL J0921.0-2258@oŒ¨€QÉ÷@2¥`À:Í~	ZõÀ;ÐNË?.?ðVGšs^G@Òܚu6¹?øÙì€nF¿îØ]Ø´s¿ïÿY<ÛÞ?ïÿd3Rµ&?‹VD"ÍéAGNbcu@½ñ‰7KÇPowerLawNVSS J092057-225721?ïó$úWÂ?qÙ,Nj?Yõ¶,R?qÙ,Nj?溜<^«?—Ò	ftí×?†0äå¢{?—Ò	ftí×?ï0Éã¨?'€!hÿtŸ?™üÅBÊ?'€!hÿtŸ?ïí©+2å?\*Fìø¸?bVÔ³Û(?\*Fìø¸?ïóæUIé?iæ±s–?X3VAž¼‰?iæ±s–?ít'¢TS>?Á†ó9H *?´[rî§@‹?Á†ó9H *?îÛûØb?›-sŸ—±ù?¢@O²bÞ?›-sŸ—±ù?ïêBwÉ»?p²Ëןݭ?eí½g:?p²ËןݭAGN3FGL J0921.8+6215@cúâ~@D'¿ó vÀ8݂ßBñÀ;ÏùrGE9?çþRåÄÚ)@ñÚbâx[@–sßË­¿âxõ7'«Ê¿æÀ¯e2ߦ¿å4eè'%1¿ê
,ZÉGAGNfsrq@''u%FPowerLawOK 630?ïáú'>Í?®̕­?nmÙFŠ­?®̕­?ïօ¤>'?"'"æÿßç?t½~/@Äp?"'"æÿßç?ï‡oßG4?"£¸
ÛÂ?Ž$;ñoZ?"£¸
ÛÂ?ï×6³£ä?UÇƑ–I?td¦°hº?UÇƑ–I?ïþ"BVU'?,HêÈÄ?&ËÛF-	­?,HêÈÄ?ïùF}gà?©þÈèÿ—×?`×0S	?©þÈèÿ—×?ï9T?ŒÐž¹J+K?Œ±¹ «?ŒÐž¹J+K?ï%ô'Úw?Š>
ÃÍ5?›_átÌ&?Š>
ÃÍ5AGN3FGL J0922.4-0529@m¶<ßï¿@@=èKŸ:ÃJÀ9°)3ÕðbÀ;±m'ª'?¸djÛ£@£ûùá@Y ÿ~û´¿ä&B×7¿×§¨%"¤¿ãÃÍZøZ¿âÏ1,·‡ÛAGNfsrq@"o=<64PowerLawTXS 0919-052?ïÿK1gè?ãMfñ~ì? .Iñ'?ãMfñ~ì?ïՁXI?†âJòÉ^ú?u?SéëMb?†âJòÉ^ú?ïê8È?ì¡?lýÝ¿e¿?eÇ7ôMnB?lýÝ¿e¿?ïë
Âü"f?G¤J¥ã?dõ<ínv?G¤J¥ã?ïþtœÆ0?)Ëz/'i¦?.˜´]µ?)Ëz/'i¦?îöœA>¹¤?±Oð°¼&á? –;ê\—À?±Oð°¼&á?ïßè\dÑ?vü(ö†œ?pÑ·C«Ø?vü(ö†œ?ï"¦]×4?ˆ@à'ÅW?›«4Vá?ˆ@à'ÅWAGN3FGL J0922.8-3959@p•É 'RT@ѿÀ9ŽaêÖ£À;n©›o\¯¿ð`ëeU@8¶*@žlŸ~"¿ë@†NÒ寿ãÃ¥×?—p¿ëõØùù"8¿]Í­"Å–ÅAGNbcu@|ºÓâÖ#ŽPowerLawPKS 0920-39?ïûu½O	?Eá&ÕU-?B)
ÀÁl?Eá&ÕU-?ï¾ë†)
?Š;fÆN&«?€E|F¿X?Š;fÆN&«?ï£_9M)?{%ñ®'ùì?‡(:µQÑ?{%ñ®'ùì?ïÿݓ͉>æoNÚÄ>ñ6îÿ4">æoNÚÄ?ïáÿË
N?tP}b€¤'?n5
º[?tP}b€¤'?îSÊ8âŽo?¹¹ÚÏkU?ªÃ\uFµ
?¹¹ÚÏkU?îö,ƙ?–·wÆ£!Š? Ÿ¿Án?–·wÆ£!Š?ïûï!ú£?BL…ÙZ€?@C{ÓÌŵ?BL…ÙZ€AGN3FGL J0923.1+3853@füÜ@W@F´ a3÷À9Ï¥ôïpÀ;Ðbƒ'Öß?×â
ˆçg$@:–n*@,À'wé¿ê¦×>ã!¿æ±ÁäÄíP'•
¶	¿ïþiWVAGNbcu@},|;OagPowerLawB2 0920+39?ïúšw²`‡?BŒä˦µd?E–"HE'¼?BŒä˦µd?ïÊA´;?†ÈMfY3?zß%Òf?†ÈMfY3?ïœ2Ǟ:?€{?Ç8?ˆó|ˆ
Œ?€{?Ç8?ïCßЂv?u3PË-À?—"ê—çR?u3PË-À?ïöúD!¤?RгØ#]ù?Rx@oè?RгØ#]ù?îØÿ…?´¥MÞ®lR?¯wK?´¥MÞ®lR?ï…f˜:?ŠÕ¡mߒ³?Ž¿x·‡ýK?ŠÕ¡mߒ³?æÓÂÿ]\–?³u¥¸P?ÒXzEFÓ?³u¥¸PAGN3FGL J0923.3+4127@f‡Ù!…Æ@F·>À//˜À9cöHòÀ;ȉ¬¼Œ?ßϙ'2@äNô"Í@	3€
&u¿Ü'èJñY¹¿ä–'˜ôX,¿äèZÄFÁ¿ä¬£b¬XÊAGNfsrq@Žåký´Ì%PowerLawB3 0920+416?ïÿ²cG¬?½AÐvkÃ?"g¥2ñ?½AÐvkÃ?ïàÙe¦;Ø?y»M'ãå?o&šg'—¶?y»M'ãå?ïÔ]sèHî?xâõ¹n6?uÑEížù0?xâõ¹n6?ïß7Ox7?NÍ1Sê?pdX}CDr?NÍ1Sê?ïþú;°'?!Ô=ç? _~&"Í?!Ô=ç?ïМ mÅ?©HWíÞ²?œEì}ªa?©HWíÞ²?ïaƒçðX‡?ÚD+>wS?"σ=!%?ÚD+>wS?ï
ÄJd?Š7sÄ#Ú?ŸþG'ÆOw?Š7sÄ#ÚAGN3FGL J0924.0+2816@hÛZÀ?ö@F7¿Ý/ñÀ9Æúû´@åÀ;àÂ=&Ò¿êƒ
^Ü7@LÒõÛ¹Ð@^`§"¿å³|ZÍ	¿èÁ­cÈHÑ¿äV&²h¿Ô¿ä™°…™\ˆAGNfsrq@€Ó>ÿP3PowerLawB2 0920+28?ïÿï¶ÝÍ>à%7S>à÷4Í_Þn>à%7S?ïánƽÈ?ïž Ðy¼?n'ãt[€?ïž Ðy¼?ïèR>¸?tÿ1î[?g­rý>'Û?tÿ1î[?ïÿê]£Áˆ>Ö3²ò]½>å¢W¼kÅÄ>Ö3²ò]½?ïÿñtÌې>ݽøԐ=É>Ýê3· [>ݽøԐ=É?ï9ÒñÌWÿ?¯WÉ¨±ä?˜Å¡ÍT8?¯WÉ¨±ä?ïíº.(?oZ›º­¦Ç?bñþqÌ×M?oZ›º­¦Ç?ïÿA¿›"y?¶™êQÎË?ÈC–\í?¶™êQÎËAGN3FGL J0924.2+0534@l\
á'6@B'"à4êÀ9ߔãQsÀ;¼Tdc¿¶¸¤®c@,ÁL#å@q·€	z¨¿âwˆ¦Ç¿í3m³À>ý¿½Ç¡Р¿Ø~.ð"ŽSAGNbll@‹ ò×sPowerLawRBS 0771?ïÿ|Vµ?ó¾mÁ? ø°¬2?ó¾mÁ?ïà"ûOA1?H°ç½ÿ?okœÇ?H°ç½ÿ?ïê\³<áe?g.k{¸­è?e£LìYê^?g.k{¸­è?ïúÔw?.
•ž³?D¯¶ë© ?.
•ž³?ïÿ_:ðcL?^t Ík?Ÿ¢»'«?^t Ík?ï wÈþ$ø?­®:OЉ?›ñãªüò?­®:OЉ?ïоo£E?{P¡¸êr?w ÈÜ5{?{P¡¸êr?ïàp›.Ö?d°:©ùÕñ?oè3VÊ?d°:©ùÕñAGN3FGL J0925.6+5959@cZV`^åi@Eu@ýAÀ:¢,nóÓ¢À;öÓ)ÞÛ?¾']Ç»"@PûSóÈ?úq™ O–@¿ïÿ½Îc?ïù\•W?­¿Ô¯$Æ3¿ÉÝTâãîAGNbll@¹ÏÎÙ‡+PowerLawNVSS J092542+595812?ïÿTïp·?JœµÁÚ?b
9Ó¢v?JœµÁÚ?ïÚG…êT?‡|]AÑ;?rÜ=$CX?‡|]AÑ;?ïãÞO'J¬?cmV÷†Ï?l!°±
«œ?cmV÷†Ï?ïôöo'?@҅Ïðü½?V –gþÉ?@҅Ïðü½?ïþ™ÚË×É?!àÁÀÒ?&bW‡mŽé?!àÁÀÒ?ï%ÂÝÌ?«ªÞ¯Ú?›G§môxƒ?«ªÞ¯Ú?ï߆zzfñ?qNÿ§ "y?p<ÂÄÜK™?qNÿ§ "y?ïµw´Ó—þ?wg®')Án?'¢Æ¢'t?wg®')ÁnAGN3FGL J0925.7+3129@hO8`™Ë@F«×à&EåÀ:å? §?uÀ<"6;%oü¿ÄXI÷RÕ@9.oÜ?ÿõ÷áMR¿ßù¥»ïb'¿ç>¥Ã¯¨á¿ºø
é˜é¿æÍXðýAGNbll@¥£…zxl"PowerLawB2 0922+31B?ïÿQ&ºe?mAÁ‰?Íû;ӏ?mAÁ‰?ïÛàÁ@Ÿ?fïëcO€?r¹!àž?fïëcO€?ïÉMµPÀs?€çgy&‹?{Y%_.êq?€çgy&‹?ï÷2ƒ2¥?;ü¤Ôލu?Q›ÿ+à?;ü¤Ôލu?ïû9 úO×?Hk-ü…ö?C|ÝÞ?Hk-ü…ö?ïځ@\?°Hé+Œ?Ÿ\dª°Šz?°Hé+Œ?ïræ+e?l%³'ê?'£:š?7Í?l%³'ê?ï¼H&gü?yRFܣӆ?€þ-ûjç?yRFܣӆAGN3FGL J0926.3+5409@dM…@FA-@F	Øà†8À:°ÄŸá§À<'ªoª²Ç¿Ü¿¡26«Z@À§8¾o@£¿bV¿Ö[A?÷x¿åuœ#âˆK¿ß2̜ț¿ä÷)攅DAGNbll@¢³'䎊rPowerLawNVSS J092638+541126?ïÈêö60F?²Ý\´XY?{Š"Ã;±	?²Ý\´XY?ï⭛ülÅ?€~På	'q?mRcט;K?€~På	'q?ï°¦ÀÀòE?‡=êtd?ƒÖOÏkx¢?‡=êtd?ïüšŽûÊ«?%ø4>ØP?;+‡²¯>?%ø4>ØP?ïýL}B\,?>ê/úí?5œ"Ï8û?>ê/úí?ï#ïv
?²r\-._°?›'5ß`?²r\-._°?ï^/ᢥe?''í]˜Ã?":ƃév?''í]˜Ã?ïÒl¢TW?oYwn
D‰?vÉ®û¤¨K?oYwn
D‰AGN3FGL J0927.9-2037@ovýç!@5kjК¸À9 ~¶¿DNÀ;»Ý:ZM?ݗ¿.©‹ª@çk›¦ÿ@ìßfØQ¿Ý@º–z'¿çVá®ä¸¿æþš­ÉZ¿æ¿þ½à ¿AGNfsrq@‰zúKâPowerLawPKS 0925-203?ïÿšïôL?†RÓ"?	DH{Ž-?†RÓ"?ïÕxTFö?'^Oão?uCÕÁß­?'^Oão?ïÛ[\p"?hŽ‹Á8GÜ?rRQîIž(?hŽ‹Á8GÜ?ïõÈÞí?4j˜jŽò?To×àóf'?4j˜jŽò?ïþÇJÅ?(qªrÒ³³?#‹ZÒzúI?(qªrÒ³³?îïςx"?²sØôž.?¡Õ?²sØôž.?ïVˆ80À?'
l˜ï ?•.ÿØùçô?'
l˜ï ?ïĄÐpª?jŽ'-ÿ&?}½—É_'æ?jŽ'-ÿ&AGN3FGL J0928.5+4048@f¤4?¢­?@G5Ôÿ¡5oÀ:¦xmÏç4À;ø˜‡Jâ|¿¬»t3Ž<@
y$nŸDÿ?ýz¹>ÐuN?æèæ˜ðI¿Ìú\ßÌPH¿á+9/²±T¿ÄÔ+j*ÚäAGNbll@¯Ö'@·€4PowerLaw1RXS J092837.8+404858?ïþÔFò5p? ijžC,K?"»'¦øjŒ? ijžC,K?ïß<	q?©Põ$ª?p|jêC¨?©Põ$ª?ïÒ¸W17?sÀÝÑe•?v£ó¿É¼Ê?sÀÝÑe•?ïù_«·?6 ÿãËp<?K—÷'‹«|?6 ÿãËp<?ïüa" ŒE?;>4êZh"?<óeRí?;>4êZh"?ïü5"Õ?±ßÿLAp:?@t4;c?±ßÿLAp:?ï¤Êõ(­ì?…õ"¬RXè?†ÍB²dé$?…õ"¬RXè?ïµÙc¼›…?{FÒ¾{•À?'‰§	ªÏ?{FÒ¾{•ÀAGN3FGL J0928.7+7300@akO¿ÆT
@Bwa_–hÀ:z²YƒÿÔÀ<
Մ+sK?ä\PZáM@
¨œÕä"ª@T¼ù›¿îeó%•Õ"¿ÚR#îò''¿ã'Å&W$¿éOÆD{
AGNbcu@xÌsBí»ZPowerLawGB6 J0929+7304?ïóH0½¯p?cž~ãçA×?Yožy¢`A?cž~ãçA×?ï?㨹û—?˜+çwc‡æ?˜Šì0)
?˜+çwc‡æ?ï_‹¥Ýl$?ŽžýXFB?"‹GÂ"?ŽžýXFB?퍫¤³þö?"

‡îoŒ?³'¢Û©âÒ?"

‡îoŒ?ヤðè_û?ŠŽ'°Z?€ZÃÌM(?ŠŽ'°Z?çÀäj­¯?ɧvÅåÛ?Ð~7ç*¤¢?ɧvÅåÛ?퀘ޫ?¥²ÿþõ¶G?³û9ñB%?¥²ÿþõ¶G?àÁÄ%çι?»Èµ³MV?Þ|w´0b?»Èµ³MVAGN3FGL J0928.9-3530@ppŸS @&xwàâ-‡À9Yp×ÙpIÀ;ˆÛýÂ8?¬í9ŒÙ@
Ööz°@>5_³Cå¿ê)ýêÑðx¿æB]ÌJ,/¿àF–½Š¿éÎÁb‹eAGNbcu@ƒBH´9XPowerLawNVSS J092849-352947?ïçúnàLJ?i$dxÜ%?h'=ðEŒ?i$dxÜ%?ïœT4	ÇÕ?û†:ð€?ˆêóý¦À?û†:ð€?ï\+þIg?‰VV]=?"z€6·›9?‰VV]=?ïE˜5Éï?zº@GÙ?—LùJ1¼?zº@GÙ?ï"ÝÈÑG?‹ø°Ñ$½}?‹ÄÙvD?‹ø°Ñ$½}?êÐ2¯ ¥?ŵñuðê[?Ä¿5C}n?ŵñuðê[?íw€y¯eÖ?£.öÎÙ
?´Cü4<ŸM?£.öÎÙ
?ç–ºrà¦?µº?
ê°?ÐÓü‹>´?µº?
ê°AGN3FGL J0929.4+5013@dõߨq¤@F¹!¬ˆŠÀ9.$I‹dMÀ;7p¯•"?¿káÝL™-@ñxŠ|E@Pàc, ¿ãI&¢ßœ¿ä㹺e/ô¿ãþ 2K<û¿Í½dqfAGNbll@"{ק†Â'PowerLawGB6 J0929+5013?ïÿÙ­ÂÒ>ç&9řs>ó)Ê<—L>ç&9řs?ïÞðOL³&?ƒtðÖ ?p‡ØE¸±6?ƒtðÖ ?ïój°Íè¬?Wn]úÙ(?Y*ž÷?Wn]úÙ(?ïûøZ#?)ݹ'L_?@'Ù: [?)ݹ'L_?ïÿâa<8ž>ç­/)‰J>íž×D†Ðë>ç­/)‰J?ï"‰"xSŠ?±–dP¤˜?›®Í'­\¾?±–dP¤˜?ïñZ^¬nð?lü‹F–^?]KBÛ\0§?lü‹F–^?ïÙL1(cn?h ÖO(?sYç|Lhü?h ÖO(AGN3FGL J0930.0+4951@e§€w‰¤@FÐ<aNÏÀ:h÷´×ãÀ; õ§·iŽ?çê¾±kž@ðÜ¡›?÷&€®ç	¿ÔâªÂêSy?ï…Þ7¿å²6ĕÏ=?Ý\–æ®A¿AGNbll@Ì=ˆr° ÅPowerLaw1ES 0927+500?ï÷ä}˜‡ ?S9Ðzé«?P7iÊ
z?S9Ðzé«?ïÜÓ½NL?'³9kò?q–!X*¢?'³9kò?îÚ¶'ÄZ…?—mî•Ö]É?¢T–á&¢¶?—mî•Ö]É?ïå_îR-Ÿ?d~âYSg?j Òî('?d~âYSg?ïʝ|ÊxV?|¸½€éqa?z±AŠEµ?|¸½€éqa?îÒ7)"U1?°©NÇ?¢Ül/ç?°©NÇ?î,úý¦x?¤%ÎÈYÞ?­>°P%˜|?¤%ÎÈYÞ?îàžýAðÌ?¥ó<œ?F?¡ö(qW>?¥ó<œ?FAGN3FGL J0930.2+8612@_'‡aˆ±@=ƒ¬ßÇ{TÀ8õ̏+\À;¥÷´#ì?äCÄeþ•$@,1â%O@xF€B²¿ÙúA©\t¿âœ‹ó1e¿å"Lu¿á\b'áÚAGNbll@Ž÷.]á\§PowerLawS5 0916+864?ïÿy+E?
Om8ד¨?Üø@(T?
Om8ד¨?ïÍ:€"tÄ?‰1BVâpë?yb¿ÌãåÄ?‰1BVâpë?ïÅÅ:Ëò¡?|Î/ጧå?}b›f‡x?|Î/ጧå?ï´>#~"?dys›Æ?'ð@¿C:?dys›Æ?ïýû.›/,?4iÀ"´Â"?0&‰…Ïš¿?4iÀ"´Â"?î´$ý1æÏ?±
Ãæ§Çã?¤½°,á"?±
Ãæ§Çã?ïwP-ÜB?öæMć?'údËá´?öæMć?í®E«¹_e? èôºke?²Ò£~ßT? èôºkeAGN3FGL J0930.9-1904@o^à?pX@6÷Û ¥&–À:‡âÀT†À;ȋfÐïq?ñuõjzÈ@
>ä'åp2?ý—sŸ4
N?ï‡HvÞ¦?ïj#hÿŒ¬¿ÙÞÏuÀîÀ¿é"KaiýPSRPSR@ªLæ?PowerLawPSR J0931-1902?ïΙÕöäp?"턹så¼?x³ù(?"턹så¼?çñ¥¸ûxv?Íæùåšà'?дŽ	?Íæùåšà'?îë©.7ý?•Ü…œc?¡Em!µ0?•Ü…œc?è;ÇÊë‡^?¯Çìk¸/¾?ÏàÔQâ‡?¯Çìk¸/¾?ïEk¶ÿ¨d? Ž†×OQ?—R‰%2]ƒ? Ž†×OQ?æ;Áv¤Äg?Ï<í=§ø¤?ӈ}¶w1?Ï<í=§ø¤?éðá¦cE?¹ƒú2üû•?È<{•frê?¹ƒú2üû•?à}æè¬Ò1?¿»ÊÏz.Î?ß2.¦[Ÿ?¿»ÊÏz.ÎAGN3FGL J0934.1+3933@fÝ]¿Î·‰@GÅ)ßÍZ'À:&æQÙ¨À;õ¯}0­G?ê·ûקFU@Žµ‹è@8RÝk¿Ý¥ø³ÁŸ-¿á¢¹䏿ãhśwŒ¡¿ìÿÊKÏGAGNbll@*÷ÎÙ‡PowerLawGB6 J0934+3926?ì¢oÎïç¯?µ7ŒwžÒQ?ºìˆ€Âˆ?µ7ŒwžÒQ?î2²1•ú(?¦¢¼.:o?¬ÔÜæ ]ƒ?¦¢¼.:o?ìÖàmØÃ?£|œá19²?¹Hÿ}Ûg?£|œá19²?ê­Rñ6?™qQߘAÛ?ÅJ´;'ë¤?™qQߘAÛ?åwœ³÷¶'?ɩᡁV?ÕƘ"²?ɩᡁV?ã
·"8¢?Ì,¡ÚÁé?Ù䑻ô»?Ì,¡ÚÁé?å ŠàÕT?½C»°^œ?Ô¿ê>UY?½C»°^œ?ÓRfBé1?¯JöËZ>?æVÌÞü‹h?¯JöËZ>MIXED3FGL J0939.2-1732@oe'@š$@9v·¿õMõÀ9Ÿlr"À;§þ#†íÅ?ëÉï"Å@ß@V‡7Â9 @(Nß·
C¿àÎ1ÏX¿ãmt‡¼Lw¿áöE"㟿íËaè¨KAGNbcu@;µsëPowerLawTXS 0936-173?ïß]{Ïô?R}gh&?pQ@,Êr,?R}gh&?ï»Z¢@Æ?‡rövý(?)Wxs†?‡rövý(?î›*ï©ü?˜<\zõØ?¦MQ¸"D?˜<\zõØ?ï1d´_˜—?sgo±ô
?™ÓipQ(?sgo±ô
?ï¢qä–9Š?ˆÇÆLJåþ?‡c†Ýá9o?ˆÇÆLJåþ?îA
e£a³?³$Ä]T/?«ïY¤Ï?³$Ä]T/?ë'×;CUž?®	)$Š¥•?Á´£ò©‰?®	)$Š¥•?볊Ÿ?¤ýÙ|a3?Á3áՃ»È?¤ýÙ|a3AGN3FGL J0939.9-2831@p;vm
J@1Ý!ŸŒø¡À9s£Ô…þ²À;¥7†
¢¿¼gù訏E@…®	Ïã@Åt®¶â¿è_ä°Ëö¿ãe€ûñ†¿äÞn´ò¿ïÿ¤vЎAGNbcu@"3Ì/ƒ{JPowerLawTXS 0937-282?ïü–Üzê­?DúG½Á7?;I@«`Ä?DúG½Á7?ïƆFM
Ç?†'$#î?|¼ÜÙye?†'$#î?ï~¹÷ï?ÐÏ6K?œð=Íèl?ÐÏ6K?ïú
ڀ‹ù?2э&&?GȖﴛ
?2э&&?ïúCdG—?P§SWG9ý?Fòo½Šâ?P§SWG9ý?îïËތ?±Òx.Ž(?¡CɆÛÍ?±Òx.Ž(?î$
‰ñH?¡Þ{òzím?­¿WqÀ‡{?¡Þ{òzím?ïÌØH´'\?o1ÜzK–ó?y"Ûµ	?o1ÜzK–óAGN3FGL J0940.7-6102@qGÿÞrÀW MRnÀ9ƒúNw\À;]¯"­¡Ž?ïÄ*×]ä@~ëÑL@^d¿9a¿Ód5Ë$<\¿ãÔ/5]ì¿ê"'ƒöo¿êb-à@¥•AGNbcu@‹w—á2µ_PowerLawMRC 0939-608?äúݸ¼¬?чžÞ¶&?Ö
DÚ†§?чžÞ¶&?ê!çÇW ƒ?À…«Š Ċ?Çx`â¡}ò?À…«Š Ċ?ì9DRGþû?¨€2M+Ã?¾5ÝmÀ*?¨€2M+Ã?éûۖqτ?œ=Î]>Ì#?È'¦8Áñ?œ=Î]>Ì#?µèP=¹?Äü×êÀ±>?ëR…Ü«ð'?Äü×êÀ±>?NJ»z"ñ"?Äà—³˜ý?êQ!ZÛ?Äà—³˜ý?Ü+ÙŒ)'?¼©+)pß?áêp¹ë8?¼©+)pß?Щ6¦Ž?¬üÉMh?ç«~õd¬¹?¬üÉMhMIXED3FGL J0940.9-1337@okÿÚ@@<g®¿›‹âÀ9«Væ—À;±gž?ÙыÇ㝸@V¹"
ä`@EÜѹ¿áÙú£°Úå¿åû¬'œ¿è'º+×Á•¿àf>"z~KAGNfsrq@‡³ÀÁüPowerLawTXS 0938-133?ïÿ\ÍDŽË?³¿ê0²w?fEê
'Ñ?³¿ê0²w?ï×^œK-Y?"(k$Ý?tP±ÐË?"(k$Ý?ïàjoÏ4 ?bÅP6ER?o•Ð`^?bÅP6ER?ïþ1ß 6?zãïèÀ?,âØ~êh?zãïèÀ?ïþšÇ?ù?*5µ#²?&^²ïßä?*5µ#²?ï…­ËÍ?²õ]Ê…?JA^ój?²õ]Ê…?ï'+Ó1Y®?ˆL{fz?‹u,Ê\‡?ˆL{fz?ïöjF›?HâI¼,°©?SÿçblŠ,?HâI¼,°©AGN3FGL J0941.6+2727@i$(?NÊh@H
÷Ÿß-øÀ:!>ºOò‡À;øgÕÒ/¿ëŠÝœ±Y²@
í1™*^@õíHû¿æzv×ÞßÛ¿æÆ(»,‰¿å'¬í€Ã׿çÔ`hå5"AGNfsrq@†GïÝëÙPowerLawMG2 J094148+2728?ïþŽÃÒ¨.?&"ˆ¦%"?'¿ÓÔ£½?&"ˆ¦%"?ïÝFhUe?€ån=–?q\˳¡Es?€ån=–?ïË󄭵l?m)5˜e*?z=²Ä2&?m)5˜e*?ïûF¹¼"ˆ?2?ê f'?B匀ŽÖ?2?ê f'?ïý^†´?7Æ7n€‰?7]ì»Öõ?7Æ7n€‰?ïNLÝ0û©?£λzÅ?–6dVpîã?£λzÅ?ï\ƒ(?X]7‰FJ?"|žm8Ê?X]7‰FJ?ïu×ÅÏ,£?Šjz–Jäé?'EDb"?Šjz–JäéAGN3FGL J0942.1-0756@nnY!…Æ@@(àaÕÀ:D"ÐÜýÀ;×Ê0:Zo?î¢Ðƒ6@ʂٹš@@‡}?pÙ1?ïþª'[c©¿Ø9î'N¿äÍExZ.˿䪀;ú'AGNbll@œtJŒL˜PowerLawPMN J0942-0800?ïÿˆr#ö?HɍðV?
ãqŒÝx?HɍðV?ï×N?€+Žýs¸?tXòk2,?€+Žýs¸?ïfžÇÉD?ÿ€GEá?",'Æ׍?ÿ€GEá?ïÀX½±Pð?bŒhËë ?Ó¡wÝ?bŒhËë ?ïÿBÝ4y?øIy"ôò?¿f@Mþ5?øIy"ôò?îç—iq;_?³[£îöÝ?¡†‰hc?³[£îöÝ?ïB¤0åY?"eA-—Ÿ?—«¸+†ë?"eA-—Ÿ?ï
!õ{Ë?-ò]~V	?ž>»È/¾?-ò]~V	AGN3FGL J0945.9+5756@c"`RP/@F¶¬@eJÝÀ9§#Pg ¡À;þEE"n¿ã3ÿ‹æÔ@–K Kz@£	ÛØ¿å_Ð˒˜§¿á·ڌÿ俋8áP›¿ç>eðŽŒºAGNbll@‹ S@N¤©PowerLawGB6 J0945+5757?ïþíûp¤?1ån<`¬J?/±"ßÚ¢?1ån<`¬J?ïæÜÇ°r?puð|¿@5?i#8PíÅù?puð|¿@5?ïÛþ—äÒl?lú<ò!¹š?r´+ÓYå?lú<ò!¹š?ïúx"ïÄQ?5z~¯8ì%?F­-à–Á?5z~¯8ì%?ïóŒüAp?_mý¿tþ¼?X濽žÊ?_mý¿tþ¼?ï=^L]óó?§e¹"é?˜T6mbIš?§e¹"é?ï"ÑÂf'¸?Š'á>sÙ?‹X·¡ù?Š'á>sÙ?ï"MV8à‹?ƒ	VKTQè?‹,ªqÇÝ>?ƒ	VKTQèAGN3FGL J0946.2+0103@mlÀ
¡©@CHEßÞ!‰À:•Rh' YÀ;¹Ã›Ë£?ã¤aöÑ>@ëréV›B?ûÏ¡‰Å?ïù«±~Æ¿ïþ±²{N?ïñ´Ï;MD?Ä ¾seàAGNbll@¿F?PowerLawRXS J094620.5+010459?ïÿÏ£8K? ïÍ@s$¹?~"1q? ïÍ@s$¹?ïÝÿ¼'&ú?wJwŽˆk?q!à½Öù?wJwŽˆk?ïħ2o¥?}Ãä#‰$µ?}¬fÌüì$?}Ãä#‰$µ?ïüE€'·}?5¸¬Yj?=Óû÷â?5¸¬Yj?ïý¡­~Ë?<ê­Ç•?2ò"|#­l?<ê­Ç•?ï$_½Ö?«»P^U'?}.àÛP?«»P^U'?=[Þ¬?ƒ»	c³Ö?‡Y°¶ÆÅ?ƒ»	c³Ö?ïüÇ}Ž?B€Þû,b«?9Ç-§å?B€Þû,b«AGN3FGL J0946.5+1017@lïàÎ'@Eµ'ÿùJÀ8­@)»»-À;€¿®Y?ó|
‡ÃXZ@	‡±d¼m@©Ç`&[^¿â¸Œ4<"¿çÑëë1M¿è£:µ¼¦¿ç¥ÞvdÙAGNfsrq@j—Oß;PowerLawTXS 0943+105?ïÿ3X9?1œì)yj?Æj–F=?1œì)yj?ï¹öl¶ë?ƒb»ÁI§b?¾'e'19?ƒb»ÁI§b?ïÈ	Ï6´r?kàËÌb•?{ûsÄä?kàËÌb•?îÃy)À u?|sÉÎ]?£ÈmeµÆ´?|sÉÎ]?ïý¥éøÆj?7Lº_¹+a?2бçå
?7Lº_¹+a?íðaô´æ?´¡a@
&â?°|ðX§'Õ?´¡a@
&â?ï´HT‹%@?ƒ…´Á²w??'íêØg;ú?ƒ…´Á²w??éu)îø?°~òõ¢y?Ê+XDû¯?°~òõ¢yAGN3FGL J0947.1-2542@p.W /µÐ@5¯ãˆÀ9sHÌølÀ;ø˜,²?Ù¯ËàÏ»@$ko9Ê?ÿ30ßEö.¿Óø«oQi¿ß6N.í%¿ÝV=Fåö¿à겆$œÂAGNbcu@¢%'@·€4PowerLaw1RXS J094709.2-254056?ïüWCU6¶??:Ñ8å?=EçæÌ??:Ñ8å?ïÃD@T§?‰UzÏ·µO?~]ßßB(?‰UzÏ·µO?ï܃Gêó?iQ¨|&`?qø¾dI–¥?iQ¨|&`?ï®ÿ—zZ?a¸S壑ú?"@ 	"<?a¸S壑ú?ïâŶÇÁ?oœ›ë·?m:I"@ñ/?oœ›ë·?îƒØxbÎh?± "O†•?§Âx{Šç"?± "O†•?À0æ?†šÕ''?ˆûÞcb?†šÕ''?ío rŒö"?›r®Å¼?´'üj¼dß?›r®Å¼AGN3FGL J0948.6+4041@fžP >cé@I+ŸÀûÀ9é ªšrÝÀ;ü	Iú¿ü¬iøÂ@ʚ‡«/™@Yÿ¿"S¿çþ€!‰£¾¿çVŒ@낚¿æINa7…¿ïÿñ([AGNfsrq@~%}keªPowerLaw4C +40.24?ïõgÐk4N?c%Ë,÷a?U0_]Ñsþ?c%Ë,÷a?ïã(ÚGgP?}lý1ß?l×%áÓÿx?}lý1ß?îÛðF#¥Í?žjSÀM`Ò?¢@ûœé¼9?žjSÀM`Ò?ïÿÏp7—é>òæß«®að>øGý¢ˆ>òæß«®að?ïý¯¶R?<>.À|9‰?72"'û:h?<>.À|9‰?ïKD/s¥?¬íۘË$?–ž'¨'Y?¬íۘË$?ïg6ÙÂê?'õnô­Ñ?"$Ǿ"Ä?'õnô­Ñ?ïù8"ÍÛH?L'ï²5q‹?K±¾QÈ?L'ï²5q‹AGN3FGL J0948.8+0021@m'Þß)@CXßÿ¯x(À7»¯ºmÀ;Y	Ó¾X–@Ü^žà@V©¡#¦£@é‹+홡¿ãøN§;¿é/2°ßäà¿ê"9Æ^•¿ïÿ
1ŸgíAGNNLSY1@pWØDЩLogParabolaPMN J0948+0022?ïè$ãü"?'¥¬¡¯úÆ?gÛæã©Ô?'¥¬¡¯úÆ?îÖš¢ûe?±–²ƒ|J?¢žvWˆµ?±–²ƒ|J?èæÓh\'?³#¯?Ìd³ö^÷?³#¯?íXéIÉçY?›º‹ì,Åx?µ8µ²úŸ¶?›º‹ì,Åx?ïÍÅZ4 e?w/c'1?yRìÏ=?w/c'1?ì;ZªV¼?Åɑ?>@?¹'
+‰1?Åɑ?>@?ìA$¥?«­íõ¢•?»%öߚÛ?«­íõ¢•?êOB$Šm?·è®ÉýE®?ÆÂ÷mזL?·è®ÉýE®AGN3FGL J0950.1+4554@e›ú€Ïž8@HÜRÿ" À9ù8¶Ç¨À;Õ
¥uoï?Û´þ,žÍ@‰}dBö?ÿ3˜Ì•¿êøÖçU‡¿ÖT©dÊD¿áf¡³¯õ¿Ï'·ïdAGNbll@£¡ÃÉîÌPowerLawRX J0950.2+4553?ïþå@ê‰?UFºÇ?!«ò,¶8o?UFºÇ?ïÞøw0Ê3?€/š1M	³?pƒÄNݶe?€/š1M	³?ïçnñû/Œ?a¸¸P8†•?h'
ە$…?a¸¸P8†•?ïѸ®Kœ$?^p›IK;P?w#¨Ë¥Ö?^p›IK;P?ïû^="e?@Е?B‡G!‡`?@Е?îÒ·.CÎü?°"°\—?¢ÔVÅC?°"°\—?ïÍ,‡â%é?|)cž©?yi»î ·'?|)cž©?íí¿ÃúÁ'?¢~/Óÿ²W?°'à—êI?¢~/Óÿ²WAGN3FGL J0953.0-0839@nř'ÿ@@óàVÀ8H.Z†^SÀ:ÙFóÚWÐ?ñ|Çô ÑF@Úú7äž?üâÝø]Ê¿ÊQʑÍâ¿Õ»ÙÂK¿ÞŽcMµÉ¿ÖtËí¿ÈAGNbll@¡Z,¿±[WPowerLawPMN J0953-0840?ïýÓ¯új?BÞ*‹x}m?1gÔ¦"Ô?BÞ*‹x}m?ïÑON­ô+?"K`âªø?wXX¡vƨ?"K`âªø?ãlù?Š|ÙÔÎø?ŽŸG+Ù9Ò?Š|ÙÔÎø?ﳚ·%ñ?a"aýì—}?ƒR*ÔóÂ?a"aýì—}?ïý²¹-ç?3ÏóU5¡œ?3'kœøJ?3ÏóU5¡œ?î·){4ºÙ?µ7óÕ×?¤hNl o?µ7óÕ×?ï[îÕ?"û+S²²?"œÞéI?"û+S²²?îâø™j…ì?ŽùU?¡ÐvlÇ=<?ŽùUAGN3FGL J0953.1-7657c@rV@ €À1‡@zC"À9ï›Á''À;ü#Òm ¿à͙—Úìd@ÛXè#•[?þ—‡€½Tµ?î"NX&C¿ÊüýRaÞ¿ØaiTµík¿â¯š
hõÉAGNbcu@²èe`A‰7PowerLaw1RXS J095306.1-765755 ?ïü¬°Äû¿?8c‹KE&?:š{à3®K?8c‹KE&?ï¸ü¯NÈÌ?"Û—è
?ÀÔ<Ëìâ?"Û—è
?ïÑnH̼K?ršª¤¥""?wHÛºžŒ?ršª¤¥""?ïø64;é2?=GQN4FÝ?O'.n-ª:?=GQN4FÝ?ï÷²lVóà?N=¡3þó?P›'&?¾?N=¡3þó?îT¸Ê?"?·œyuYž?ª´s\ë~Ä?·œyuYž?ï±Z߅È=?ümÙâ0û?ƒ©HǞê?ümÙâ0û?ïº1"HŸ?u±ˆø.sà?s·bMl5?u±ˆø.sàAGN3FGL J0954.2+4913@dôªà~Zy@HÉö`D
vÀ:©î,˜å?À;Ë¢1Ð?äL´Ø©Í@°†'¡Ú†?õM9§š¹?îwÂ%Ì:¿ã¤ähŸÑ—¿ïÂ0œÞ{)?ﰋ֍jâAGNbll@Ñ}3¥ãSøPowerLaw1ES 0950+495?ïõݐú?e&ÝíT?TDߖE¬©?e&ÝíT?ïãxvøô?~æN®,ÜT?l‡‰ëë=?~æN®,ÜT?í¯XŒwáÓ?¥/§¢pÙ?²…;œ®äê?¥/§¢pÙ?ïüö`Í}Õ?;†•o6C\?8LùS2O˜?;†•o6C\?ïé±Árj?qõÒY•?fçNmHEP?qõÒY•?ï5M¯Ø?¨+p—ž?™VJ#4™'?¨+p—ž?ìƲUs¥?¨ÇÇ}aè?¹Êo¥TbÙ?¨ÇÇ}aè?ïtR)T?¦MB(ô‰ã?'u½üJO?¦MB(ô‰ãAGN3FGL J0955.4+6940@a®+ÀãŠ~@DE…`&±EÀ9A¢e6À;Ï"כ\è?Ñ9Ô
x@
xjRWù@®#ÿ¹‰#¿ßßëÄ¿ÞTžç·4¿çÑ,ÎDœ¿ÛÄę!¥OTHERsbg@¹–¡aä÷PowerLawM 82?ïé-oyà?oRü,Ýî?fð҈G ?oRü,Ýî?ïËz9#"Œ?…¼õ40—?zBãŠj…è?…¼õ40—?ï2j‰>`A?'×Xxu?™²®Óõ?'×Xxu?ï7p`™?'[0ìö§«?™΄Pë?'[0ìö§«?ïç£"? ÝåØDKË?œîC
G›ˆ? ÝåØDKË?íBŽ¦²—þ?¼0áV>"?µëŠÈ³r?¼0áV>"?퐰N?ªSžMÈ?·K"}‹ú?ªSžMÈ?å4è½Ì²S?ÁÕzgdžß?Ֆ."f›Y?ÁÕzgdžßAGN3FGL J0955.6-6148@q»-ÿ'+¿ÀÈÙà0¬ÆÀ9…¦ a4À;dM\‰?êÄG©³@
}~
@›_¿®+L¿å÷ó4Ѫ¿â·K:Þ¿ÛY6ÿ⺿îÏ
L½¦rPSRpsr@"/<ÚQPowerLawPSR J0955-61?ìÛå‹%Ò?¶«U¢œo?¹ ×E^Ÿl?¶«U¢œo?é£Óà(?ÂM_Rå™ç?Ép°—Ã^?ÂM_Rå™ç?ì"@œ}Nµ?¥•V`VNc?»eûŠV?¥•V`VNc?éáPxT? ê¨'3¯?Èz¿¢'°? ê¨'3¯?Ûû`n)Ô:?Ìà'!Eå?âOÈëã?Ìà'!Eå?ÆøˆXÚ&?Åv£L˜+}?êAÝÿéÉw?Åv£L˜+}?åð''7?µß…01õ;?Õ°ېÆ?µß…01õ;?Õ3°y¸†L?ºæÏ
l?åf'Ã#¼Ú?ºæÏ
lMIXED3FGL J0956.6+2515@i¯?p]@Iwù jn3À9!Áû¸r£À;²#ÃS§G?ðÐój›TZ@ÒPw¹Ë@|G '¨;¿ãGXÕ6Ü>¿äãëSdoÛ¿è_EüŸ´w¿ïÿ˜µÁ²AGNfsrq@"'}At>–PowerLawOK 290@?ïöM{Ö1?UÇj5û?SeÏNµ¯?UÇj5û?ïÍJ‡§n?ôñš¾³?ypÚÜx?ôñš¾³?îùÃê"Íœ?'r'fg· ? cÁU×?E?'r'fg· ?ïMgIî¿?t#刓‹…?–SÃßêì?t#刓‹…?ïõYì/"–?]î2"ì?UL'×ҒÉ?]î2"ì?îÈ¡ß¹8›?°Í†‰-x?£uâ óQ?°Í†‰-x?íZE´rÁq?§'c…i?µ-ÒZ²&y?§'c…i?ìc:¤›?¦m°c‰?¼æ/Òß)?¦m°c‰AGN3FGL J0956.7-6441@qك @ÀÀ'{ 4hgÀ9´Ïú~¶¿À;}hq¡›¿Ó>ehIÀ@wZ!‰'@Ià [R¿å•‹g>§¿é‹åô¿å	=Éí¨¿Ó=X™&àAGNbcu@ˆ$T•*™PowerLawAT20G J095612-643928?ïýÔ[ƒÖ±?1Á-ÆQ?1]"ý±%?1Á-ÆQ?ï©·	À=?'[*Â".;?…'=´àT¼?'[*Â".;?ïˇ}‹?s ܖ³Ô
?z<9KŽo?s ܖ³Ô
?ïüØBÌ®D?$‹'F4ÏO?9=ê"äÅü?$‹'F4ÏO?ï÷öiÎ?Vj'´¤?Qø#¥'û?Vj'´¤?íRd";?½E˜‡îí?³lá›4%?½E˜‡îí?ïy*C¨ÿÇ?c£wð¥»?Ú·ŽO£&?c£wð¥»?ïÓ¶¸I™?m5~ÈŒ?vx¤£+Ge?m5~ÈŒAGN3FGL J0957.4+4728@eA¿p@IIí )k3À:¨(÷À<ÿ™¨³?åðQòċ¾@"y$én@[œ@gú¿Ùftlþ¿éÅÿýËÑ¿ïj'"?ÐÅ@CŠµAGNfsrq@}JŒL˜PowerLawOK 492?ïÿW‰²Nz?!wkïõ?ÎfÛo‹?!wkïõ?ïÛ\ÄQB?†°ÌÐd?rQõ!Fúû?†°ÌÐd?ïB]Œð`G?"˜]Õ)Z?—´NhÓ/?"˜]Õ)Z?ïðMv'"?S™Ï®ƒR‡?^áeR©¼?S™Ï®ƒR‡?ïýcjTÿÙ?JË^ªQè@?4䫍'&ñ?JË^ªQè@?îϋ&ó•?²,8øWÃ?£M H"¬?²,8øWÃ?î;'{üP?¢ ¸HÕ?¬FÖ%¬†?¢ ¸HÕ?îÈ¥ût!‡?¦°3'äd?£u KQœ‡?¦°3'ädAGN3FGL J0957.5-1351@os Æ´…@?.²˜¬4À9_ÄM¢JBÀ;ªFX©åA?öfàý0lÚ@wŸäŒ\@)=³ê¨«¿ás؉ÚP¿æY<Ž&¿ë8ÙP;y¿ïÿ"û&ýEAGNfsrq@|Ž`€sXLogParabolaPMN J0957-1350?ïéHz\v?cÖ5Ye»]?f·…~ãÂ~?cÖ5Ye»]?ï´:"¾}?ŠfMÅcT—?'ñ[W˜?ŠfMÅcT—?îb>ðÅiE?—÷N¢ò«%?©Üõa9®?—÷N¢ò«%?îꚸ¨}?€|¦÷™?¡VTxÜ+?€|¦÷™?ïÒpáó?zïËGÇ?vðÇè6ð?zïËGÇ?îcÈ?·¾Îëµ?¯Ÿ	ÊGü?·¾Îëµ?í{·1Ô?¤fëðŸ'?´"Gý'…?¤fëðŸ'?뽪èBì?¬XÀ^Êþ¦?ÃÑ	T^ôO?¬XÀ^Êþ¦AGN3FGL J0957.6+5523@cÒó@ÔÜf@GöãàÈñÀ7nû`^À: u'ÊI?øÂjž.@
ûãL@€?ýÌðW@"¿ÙNKÏié¿àšÈ0ŽpÏ¿àÕ£Ñçúâ¿âd»rv-óAGNfsrq@'FýuâLogParabola4C +55.17?éROxc>?"¦\íä?ʶÂs´?"¦\íä?Á}
Éä‡v?ÈuõÛ8öA?ë ¼†Þ#?ÈuõÛ8öA?é)ç9r?¯|sÎ@Ü?ËXc¿ÿ8?¯|sÎ@Ü?ĵø—p?¥;âÎ#¶?êÒ¹Ú$?¥;âÎ#¶?Þ~ë(¾¡?ÉíkÚ)èÃ?àûÀŠk ¯?ÉíkÚ)èÃ?ºs?}Cw¤?ɺ,·/¢?챘W'?ɺ,·/¢?ç¿ÙýÔ,?²¢í¢9¹%?ЀMÞW©?²¢í¢9¹%?•ÍI8G?†xX-‰?ïQ•¶'ï?†xX-‰MIXED3FGL J0958.3-0318@nD¸€®@C.^è¬À:uÓ|ê6jÀ;—ÛBö?ç±Ä‹_Å
@
wã'_c?ø=ÖÀ¯?¿éśžæ¿´Á¨Æ!%Ù?Õ<OÞÜç?º¹U2AGNbll@ÀºPowerLaw1RXS J095806.4-031729?ïý³Z=–Â?2`B§K'?2e0w"¦?2`B§K'?ïÛ
µ›?~8Ί]ƒ?rz¥Po£¹?~8Ί]ƒ?ïϕ˜>`õ?}ê!B¯è?x53ÐQe?}ê!B¯è?ïôI…¨:?EÚºÄ!?WmÜÛò\d?EÚºÄ!?ïù7&»^C?Hєç<?K#eg0†–?Hєç<?îûHÝá¿p?³¥ŽW`I? Kr"¿ð?³¥ŽW`I?ï®rìST?ƒ`Š+J?"cDáñù?ƒ`Š+J?ïçw´9ó?dX ÛFR?hˆá€	?dX ÛFRAGN3FGL J0958.4-6752@qû™€o&)À$Š>ž¡@WÀ9ûͅYqÀ; ô‰u?Й¼(ÃK@
áJòA¦i@§ø`ygu¿ëK"ÞK¥E¿à`–!ƒÍ¿ØP¿ˆõ?¿ãf"Ú ¨ŠAGNbcu@Ÿj(õ\PowerLaw1RXS J095812.8-675241?ïü­êÖÅk?;&+7Ü?:©7•?;&+7Ü?ïC­B³?Ÿx<íz?Œ:/"mÃF?Ÿx<íz?ïݑ¦0*ë?sVrŠ,…l?q7,âk*€?sVrŠ,…l?ïÁî;KIn?^õ5ÈÎa?â]ÊäÕ?^õ5ÈÎa?ïó&
8€?W¹—òj¸?Yõ´5Eîâ?W¹—òj¸?ë½·ËUJØ?Á"ÿö3½6?Á	 ÒªÔ¢?Á"ÿö3½6?ïªËËx—?‡ï5£ky?…x?‡ï5£ky?íø#Ðó*¸?˜¾{7
?°>ázŒk¼?˜¾{7
AGN3FGL J0958.6+6534@b82€ñ,(@E&Ÿ¦ùÔÀ8¾­µ°P•À;ÁUÊ6ðW¿øv†PÀb@ÃÖDDÓo@
@?‹0J¿ã•Ó€ná¿åÒÙõ‡à¿ä-Í÷!é¿æ®ƒZµO¥AGNbll@'º>-b9PowerLawS4 0954+65?ïÿÓÔö3p>ï&€ Yî>ö'Kél<>ï&€ Yî?ïኞvo•?cÁ8Όm?nuapÓ:Ç?cÁ8Όm?ïï~ì!ÚN?^vÒ~ép?`ÁHú6?^vÒ~ép?ïÿýT6U>°Òjá½TL>µ\Ãã¹^>°Òjá½TL?ïÿÏFàËC>ó7Á~X>ø\JÀ>ó7Á~X?ïX•'­x?¨vß2¡Ø?"í\íÊPú?¨vß2¡Ø?ïìH"—îŽ?eÏ!N úÂ?c·{˜+ú=?eÏ!N úÂ?ïÿàOái½>ô0,ÙR8Â>ï¯ôûóì>ô0,ÙR8ÂAGN3FGL J0958.6-2447@pDêŽ:Á@7pæàtI~À:
ZÜÅhTÀ;Âá½Ùà?·3Q7Ágˆ@XÓÞå@ðp¿…¼m¿á\ï»Ü¿åºH싌™¿æ\wÜtNu¿ÔnRÍF3AGNbcu@"<ùÛ"ÐåPowerLawTXS 0956-244?ïþߍ³v(?"Ïÿú=Ž?"$7zÆõ?"Ïÿú=Ž?ïÆÉL(']?ŒÑÑh'/?|›YÙ)m]?ŒÑÑh'/?ïÛ@ßTu?e.<›=:ú?r_qòG›?e.<›=:ú?ïñ&¢šãà?EHÜú)ÄÐ?]²ºVÅ_ù?EHÜú)ÄÐ?ïûål^€œ?D >$,?@jMßöÕ`?D >$,?îó+šŸ ?­
1½TnH? ÍOz'?­
1½TnH?†[
?‹^øÍ]?Œ_XÙu?‹^øÍ]?ï,oŽr
?ûLaähÎ?œ:r
Â"e?ûLaähÎAGN3FGL J0959.7+2124@jtþKZ@IQ4 ½À:[®a§ºÅÀ;äEÞ0¢_¿þ‡†AM'P@Þä‡(¨Á@) CVí?Õ®ï1%¼Ó¿ß"ç†óŠã¿ë>ãp?›+á
ÈAGNbll@ N^¸Që…PowerLawRX J0959.4+2123?ïûâÝèÍ?OåÞÓå™?@tò]ªï^?OåÞÓå™?ïâ;¨D$?Ï;ɦÿ?mèĊ–ü?Ï;ɦÿ?ï*'mÞÞP?'GÌJÛkW?š­²=Dþ?'GÌJÛkW?ïÿþ?-ï>­+"êS¸>¬	–: ñ$>­+"êS¸?ïìõ\õ	¾?l"Â릚r?c
£+òÒ?l"Â릚r?ï} è‹wË?•yíX'Ñ?[âðHԏ?•yíX'Ñ?íTÅ#W•`?¬fj67q?µYÖæû#?¬fj67q?ïÿ·×áíŠ?y™@/U?
»s?y™@/UAGN3FGL J1001.0+2913@hî^ß)@JK8_ÂÞ7À9'Ö!à$˜À;ÁCÂÍoŠ¿ô‡XC¸çh@ï1Æ̂¥@A›Ÿ®0ª¿á;™Užd¿æ›Siñ¿áhòüGŸã¿Ó—Ãl7AGNbll@"zÑhr°!PowerLawGB6 J1001+2911?ïÿççãÝ>àчšf#@>è8â—ç>àчšf#@?ïâµæÙ?|Ì#âaÏH?mJøþ'G0?|Ì#âaÏH?ïö"PS¡à?D]Äx_Î?R÷^þq?D]Äx_Î?ïÿþèJN$>–æ\Œ€>¡zTÆ]²Û>–æ\Œ€?ïÿòËÜYT>Ö4r
Š>Úh*÷^#>Ö4r
Š?ïh9Aa–•?¢*'¶âë?'ø×Ð]'[?¢*'¶âë?ïõ¸T€ñé?c×Ñ&'¹?TV³äž#?c×Ñ&'¹?ïÿöEþ"A>Ԑkç!
>Ós»Ïƒ›>Ԑkç!
AGN3FGL J1002.3+2220@jPå`A‰7@I¿f€g™lÀ:d~¡ÆÀ;à\d"ä׿ǃ'Ù6Ã@ëþ<[{@x¬ßœˆ6¿Ý]ޞl£S¿ê8Šò¿Õ2–È%j•¿èB`é"]AGNbll@"Ÿ,<žìÀPowerLaw1RXS J100235.8+221609?ïþÁ·?"fóÚV?#äŒ
ÂCÝ?"fóÚV?ïØáD7?"˜"[?söE« y?"˜"[?ï¨nKb)?"GêڑÍ?…äm1Ď´?"GêڑÍ?ï֊"lXï?^.Ê°W¿?tº¶4…ôÆ?^.Ê°W¿?ïû"Zÿï©?GY¼£%‰?A²"ÿW?GY¼£%‰?îÖxŽ Ûò?«E"Úy%?¢˜waÜÜ?«E"Úy%?îÚqs	âØ?—G<¶†é?¢XèËò6ˆ?—G<¶†é?íõÓaš|?£g–mµÓ?°QdôçÂ?£g–mµÓAGN3FGL J1003.6+2608@i"&?šIÃ@JV<ã.À:nˆö´&äÀ;ãØ$ãý¿áYZŽ/ÇÞ@
ÃNÿl‡=@UÎ 3ý¿äÜ4~]z¿èñ*,××ö¿Ò'i!à-¿êŒ²$ÒÏAGNbcu@–Ÿ­úCþ]PowerLawPKS 1000+26?ïúõD˜¾Ü?U25Lâ§?D*íiW=Ñ?U25Lâ§?ïߨÌèPŒ?'³#eÖ?p+™§.
?'³#eÖ?Ù'u?~˜]«î
(?ŠY	ÇÚ¾?~˜]«î
(?ïøh:7D¡?;'­ÜiÚï?N_ÉQF?;'­ÜiÚï?ïú–Å1€‰?I%*ÇÆ@n?E¤êä:Îê?I%*ÇÆ@n?ïÌüûò2?²vŒIžn?æ``¹Ã?²vŒIžn?ï%mVĪ?•òŽNù˜?›RPH2Ã?•òŽNù˜?ï›Í¡'"C?'Ëêfs!?‰—¢zg?'Ëêfs!AGN3FGL J1005.0-4959@qYBà°«@
Ý¿ä1À9 –6—À;W¢Õ'}ô¿í¾¾Ë='Â@
çEgée@78¿å׿é殚T!¿èrWý(E€¿ç.ϧ%Pû¿ä"0™[ AGNbcu@xÊ\|ؙPowerLawPMN J1006-5018	?ïùߎÅ^?PM"03?HÈ_RŠ¯?PM"03?ï¸uÒÀá?Ž­!¨D£?â‹M@¥?Ž­!¨D£?ï£["Ïf?|vVEé8?‡)Š–n?|vVEé8?ïý"ã_?#ôi÷¯Ê?3cxìºCý?#ôi÷¯Ê?ïØvõ2z.?x"±"P?są€0¶?x"±"P?îY%¤îü?º%P*ÃV?®m£[C?º%P*ÃV?î´¸Wä‡B?œœ—Éâ?¤´z€Û¤Ú?œœ—Éâ?ïÃ&‹/¥?uY‡túë?~lº'Ž5p?uY‡túëAGN3FGL J1006.7+3453@g€Àð¸@K6îÍ©À:¾ž\vù\À;êň4íH¿×ך3{
@@
cJØkf€?ú|R@¿Ê¿ïÿ
ç\›?ïÍ"Ê5¿ÔÄ@ٱ뿹ܦ/eY‡AGNbll@¹½è_ö"PowerLawEXO 1004.0+3509?ïþúɁ¶?ç²[ÓU? Sku6"[?ç²[ÓU?ïãÅӚ'‰?|ü`Qd!Ä?l:,b½Ç?|ü`Qd!Ä?ïÕÕŠoŸ?mtY÷ ¾…?uu+©è£?mtY÷ ¾…?ïù ÁgO+?8þNýêñ{?I|úÇëŒ?8þNýêñ{?ïþB°K.I?,³IˆŽ°Ì?+Ôû½Aáç?,³IˆŽ°Ì?ïIï:"'\?¦Ð±cçc?–´nìy?¦Ð±cçc?ïŤªÀÖ?{l,h%?}-û'2?{l,h%?ï°æU²ã?ú´ç÷?ƒÆjËa{
?ú´ç÷AGN3FGL J1006.7-2159@p<۟˜·@:ȖÀ¡E`À8¹æè¹À;ŒÕÓËò?Åò´âd'Œ@.ÁКaÁ@z›@7Ӂ¿âJ°7S¿çæ `U¿è%=ÍÒŸ¿×Æ*g˜Ñ¯AGNfsrq@µÎ;Í5¨PowerLawPKS 1004-217?ïÿ¡IL‹Z?ÓÊÀ›2?­¬Pl«z?ÓÊÀ›2?ïÛbã`HP?€$³"=Ӂ?rNŽ8~ï?€$³"=Ӂ?ïÜ[7ì?nî5¶›â?qýÒE‹6?nî5¶›â?ïú¶â¶Í?/℈ùØ?E'÷…ÿÿ?/℈ùØ?ïþ"‡äc?+€
9×Í?'·}Ž¦
¶?+€
9×Í?ï ûQ‰N?°y³çôW?‹àŽïž=?°y³çôW?ï¤$i@á?‡Óø¦t'\?†ù¶å¯Ç®?‡Óø¦t'\?ïÇõò'`d?p·ÂKÚ?| "=÷?p·ÂKÚAGN3FGL J1007.4-3334@p¾%`A‰7@1é¬ "ÚÆÀ:Ž(LOdÀ;¥¹¯¹–?ñÃv¤÷ñ"@·T?@N[ÿ…0׿ßúú¾]Úb¿èÕìÅTw¿èq…­Ғ¿ïÿ8Ýl,NAGNfsrq@ƒDœygËPowerLawPKS 1005-333?îMÍAÝg?¯NCêA{?«#.‡–¦?¯NCêA{?äõÚöíBõ?È°âOYÉ9?ÖJ%z?È°âOYÉ9?ì°7(
O?¥?÷,jîÁ?º~Gv¿­ˆ?¥?÷,jîÁ?å«RR¡ý/?¦e…A%˜?Ô©[Z¼¢?¦e…A%˜?ì,'†úÒç?À¯Ïf@×?¾›ëÈ)hÉ?À¯Ïf@×?Ç j­Wš?Ç«ñux¨?ê7åÔª?Ç«ñux¨?ä¼XQêr>?¹kÕöá2?ևO\+"?¹kÕöá2?ÃJG¿å¼;?£~ùRŽX£?ë-nñ?£~ùRŽX£MIXED3FGL J1007.8+0026@n?@OÂ@EFv¹ÃÀ:BôˆÓx¸À;Î))Äõh?×Íí"äg@²A±%@¶'¿t?ïýÙý¡¿å"­·]Ï¿¿×®O½Ç:+¿ç`n©š²bAGNbcu@žÿ—$tPowerLawPKS 1005+007?ïþ¯9M?&}x{‡ó?%x˜ÐYÚ?&}x{‡ó?ï°«àÝ¿¨?ˆmQþT£(?ƒÕÀQ?ˆmQþT£(?ïИǬ?t¶§È¨È?w³œgÆ)?t¶§È¨È?îÛ¡tb6?†?w՝­…?¢Eè¼sa—?†?w՝­…?ïûÙõÕ.Æ?S1x÷ü9?@˜)Xq6Ë?S1x÷ü9?í>`¡¼Žø?·y­+äã¯?¶úñ?¡??·y­+äã¯?#DD?‡ÄŸ¸´ÀP?Š·B&æ?‡ÄŸ¸´ÀP?è€Wt—<Ù?´<DÔXLì?Íþ¢-£›?´<DÔXLìAGN3FGL J1007.9+0621@m00ÿì·@Fÿì@/šøÀ8õ¬Á"ŠfÀ;}X¶zzð?ï½ÅÀ6@Aé;îB¾@@<`ƒxp¿ÚIÿ6Ô¿å9=–ìô"¿åÈ,Ì礿¿ág"j´AGNbll@X½p£×
PowerLawMG1 J100800+0621?ïùÁsÂg?I#—v¯M?Hú0
yç?I#—v¯M?ï­Pv¼é?"ƒXìS›v?"«âhâ¹ë?"ƒXìS›v?ï»áM&=?|æÈB™ÃŽ?;¥'L¹?|æÈB™ÃŽ?î–ßÿÉ=:?€¦A&t¶œ?¦'ÿÿüd?€¦A&t¶œ?ïì\=SÙ­?kÉš>Êá?c£Â£çBõ?kÉš>Êá?ì¼n L¯9?¸‰Ø.Ë\š?ºŽýš†:?¸‰Ø.Ë\š?îšæLòïC?œ]Ç]$³?¦Q›/õ$Ö?œ]Ç]$³?æ¤Ô¤mÄ:?³&»øáu?Ò¶V·$wŒ?³&»øáuAGN3FGL J1008.9-2910@p"íà
q@5cÿƒÙ>À:.'Gl¦À;ÄÁE°
y¿×ÑkJ¯Y@ÓÆØA/@ à"ªÇ¿ìD]|i¿ãèPÔXÝ<¿Ñ»:X–o¿ìànà]xVAGNbcu@)E8ï5PowerLawPMN J1008-2912?ïɋ‹}»Ü?váòÄpAb?{::Åú?váòÄpAb?ïÒäXڌ©?ÿ«:¯®?vÓrmWµ?ÿ«:¯®?îdûU)å?›§1ðƒ"[?©°J¯'´?›§1ðƒ"[?ïòHpËÞÕ?Fe¹å²ª?[o˶{?Fe¹å²ª?ï¢ð€Ž¹I?"£"?¬#›?‡CßÒÙ´?"£"?¬#›?ïJ–"ÄÔ?ª5í…{•Ó?ž­+÷Ɉ?ª5í…{•Ó?í!Þfþè?«Z+ZüÄÅ?¶ñÈë_Ã?«Z+ZüÄÅ?ïsËv,úV?‡Y›–ºW?'†'<ƒ0?‡Y›–ºWAGN3FGL J1009.0-3137@p®…×E@3¥Ð]óÑÀ9¾~ÝU±À;jõ2F¤)¿ò\ªÈÀù…@BN¨Ú@ÈŸ~µé¿Ë×íÇïz¿èn[ø¿ã=;þ¿àáH2¯æÉAGNbcu@'>ùrGEPowerLawPKS 1006-313?ïúÐÒQ,T?Pj"(Î?D¼·Ñm¡?Pj"(Î?ïÓT£›P(?ˆHw9³°?vU®N"·Ó?ˆHw9³°?ï£Ü—ßÉî?''Zg͕/?‡Ú
"g?''Zg͕/?ïþÅgu&•?d±W_?#©Šö‡_>?d±W_?ïê¢[»N?kC™ÞgÎ?e]ü¯Cr?kC™ÞgÎ?ï,ô!-w?¥<ʳ-n—?ša|"¹‰?¥<ʳ-n—?î…Çû+ÚÏ? 5V
¨µ?§£€N:? 5V
¨µ?ïà•$¦
×?m…dúDÅþ?ojÛ668Ç?m…dúDÅþAGN3FGL J1010.2-3120@p®Ñ`4P@4
Z?çvœÀ9˜
¨_/À;"30®ô¿Íš ;@ÔΎmìm?ù8}_|<g¿ï–`p?ØÝ|v·Ü¿±ëSBÃ#¿Ð9o•í›AGNbll@Á^vÈ´9PowerLaw1RXS J101015.9-311909?ïÿ'Î4'?×.܌±â?L~'ò³1?×.܌±â?ïÍ ؊?Œþª¿~?yoþ´á&¬?Œþª¿~?ï·4ûgób?ƒÜ—Ps?'2Á(já'?ƒÜ—Ps?ïÿnB±^>þ@á·Ì£}?7ª} ­€>þ@á·Ì£}?ïþá9–N¶? 
müù!ò?!ìcd¥P'? 
müù!ò?îö³ÆÊý?³ÀlßTÎ^? "Ïïô0?³ÀlßTÎ^?ï´]¡Š˜?‡Æﶛi?'è—¥˜ìN?‡Æﶛi?ïþ&%{(?%BiFFfn?-¤}ëî?%BiFFfnAGN3FGL J1010.8-0158@nl»À n @DÏPßìdBÀ:+î^íÌ!À;ÓN+>?ÀU¤)ó÷è@⧊Hò@	4¿zSÙ¿ãè(b}V¿æ!\?µ¼T¿ävÌsP¿è4í™1PAGNfsrq@ŽZ¬1PowerLawPKS 1008-01?ïÿ(èŠ ?t#£½?:á;Sâr?t#£½?ïؐƒñ<?ƒ[ RÛ$?sÀ7µf+?ƒ[ RÛ$?ïë°ÀÛ/š?g]"¥§æ'?dO?9n:?g]"¥§æ'?ïéÔ7­ÉÛ?HÄNI|(?f+ȉ/äÖ?HÄNI|(?ïÿMê!? ƒϒ½?V?¦Uä? ƒϒ½?ïô:
N?­:¬F–þ?Ÿ¡x¹ŽÒL?­:¬F–þ?ïÒ¸µ¤Î<?x§èäà?v£¥2hUÔ?x§èäà?ï#6p?‹ñsìʸ?ž.[ Ië?‹ñsìʸAGN3FGL J1012.0-4235@q#,ÿ§ël@&kþ>^à`À9ž9Pƒ¦À;…§ÉÞ?ôŸ^<vRî@
9""Ï°W@9nà2…8¿íytí<Ú?Üÿ<ÊûU:¿á~ˆ²S[¿î
Š°Ù¸TPSRpsr@¡S_oÒ PowerLawPSR J1012-42?¼³šÂt|?»SÙ±a·U?ìiŒ¿§±q?»SÙ±a·U?ÃlYÎ:?ȐÀWž?ë?¤éŒ~²?ȐÀWž?âØX]Üv…?´H%iK<!?ÚOODGõ?´H%iK<!?Ô G
´?¬ß]SZT'?åó/þÜz¦?¬ß]SZT'?¢kØÍ(jÂ?°ßP'?îÙBsds?°ßP'?¦nä;ÐÊ?·UaՍy?jÿÓ?·UaՍy?Í5UF™?µ×âe^€H?è²¹*®Z?µ×âe^€H?§'>Ê€Â?'Ý¢è4Ͷ?h#?'Ý¢è4ͶMIXED3FGL J1012.2+0631@mE:Kâ@G?µ!µÀ9¥"÷si"À;"ÿ·¿ÔGpõê @ +Dý5@›{Q^—¿åρZ]™Ž¿ãþ À'¿â©W'Á–Á¿Ô@ßu"AGNbll@¢$!|ÚQPowerLawNRAO 350?ïÿÉ¡ÛC?´ìÁóU?fÏú!Ø?´ìÁóU?ïàœ<âž?|Љe†ý?ocÃ(ö!½?|Љe†ý?ïîZ™(°x?`aÙÉp?a¥géo]?`aÙÉp?ïý@\ˆäb?$
5ÊþÉ?5ý´G]Õ?$
5ÊþÉ?ïý¸–E7~?1 ™ á¿?2;Må«E?1 ™ á¿?ïK¨ÁL2? /0L>–?–Ê櫲? /0L>–?ïÞ1íL?uîk²Èk?pçpœµ)Û?uîk²Èk?ïÙ'N"¢Â?j@eWë÷Ò?slXÑ!û
?j@eWë÷ÒAGN3FGL J1012.6+2439@iøn «†@K+|à%o%À8=†Ñ™»À;S=Êeê@?÷¨¤&æI@WƒsèZ@ïJݤ¿Þ;:žaw¿ä.ŸJç¿åؼUl¿ìК›»÷AGNfsrq@~M:'£LogParabolaMG2 J101241+2439?ï–ät"‹?…i[y¨w?ŠFãzU/?…i[y¨w?ïݦJGç?…=Ãbž?q,òøh°?…=Ãbž?ëÜF'`•A?¨±U`>ß?ÀŽå¶}ªü?¨±U`>ß?ïógàÜE³?CŽØï
T?Y0>46Ê?CŽØï
T?ï2€æ½?•W!Ã×Ø/?¼LsŒo?•W!Ã×Ø/?ï(~1fÝã?°lF"†¨?šð9ÔÜ™?°lF"†¨?éô{,¾q?¯ÏYÒ^?È.M:?¯ÏYÒ^?ïé›ñÒY˜?aYU£ I?fd[?[?aYU£ IAGN3FGL J1012.7+4229@fԀu@K3N?þó'À:r±ÎCÅÀ;¨¬¥åØ7¿âb¡Úà%@]lWA/u?ú‰ ¨+®¿çþ¶lÛ¿ãñðPh+¿ÂOw݇/¿Ó´í¡ÈVAGNbll@¶F¶‡+PowerLawB3 1009+427?ïÿ—6µ@6?®À›Ô."?
2_REc{?®À›Ô."?ï࿼îÞ?…o¡'Ú?oø@d
aŽ?…o¡'Ú?ïñ)"Žh?X˜I.'zš?]­ºñŸø?X˜I.'zš?ïÿdÌTÏ2?ÅêWûòR?fmp|^O?ÅêWûòR?ïÿ‹ÞÅó•?¦$Yô 0?
?$œÃ'?¦$Yô 0?ïVS*8Qš?¨ÜÜ˃³?•5š¾6¼?¨ÜÜ˃³?ïñª¢Uä?a«‰:áÞ?\ª»h>n?a«‰:áÞ?ïúän˜Ó»?A âóDÏ?DnF"ó£?A âóDÏAGN3FGL J1013.5+3440@g̸`™Ë@KÃC hÀ´À9Á/¡®;À;ÐsۍZ¿çنO@  ïX=@þ¸ Bj´¿áLã1£¿êt@;%è>¿à
ù¼«'È¿ïûàˆìMFAGNfsrq@'w:'£PowerLawOL 318?ï	h_k?ÅÜÉïø¡?žÒü¹9ø?ÅÜÉïø¡?ïßqj%®?"±nLÝ?pGJïHìé?"±nLÝ?ï½\²2˜?q['G/}?€¸¨ÚR'?q['G/}?ïúñªÊû?2'(·ùy?D9SßÏv×?2'(·ùy?ïþQxT6?0³«z¥*o?*ï	å"a?0³«z¥*o?ï@÷E` @?®Œlp?—áMÀ
?®Œlp?ï¦eت"+?ˆãKC"7,?†f‰Õ^õ7?ˆãKC"7,?ï³
Å£§?|CÍ+Õ±?ƒ=zßÅ"	?|CÍ+Õ±AGN3FGL J1014.2+4115@f\ÍÓØ@Kwÿ´€¦À:a)ë‹ÔµÀ<‡ð#éê¿ÜÅèéMY@æ?Ns@c¥ÀnoŸ¿¼UÙü5E1¿åìÖÔà!¿âì/a¨¢²¿éKÍ&¯AGNbcu@ŒÆŸ@¢‡PowerLawGB6 J1014+4112?ïù;ÊJUS?\VŸ·Qy?K֕>ó
?\VŸ·Qy?ïÜïÎÉ@?†«Æ kx?qˆ«ÞÑ?†«Æ kx?ïb5o¬÷?È-'U?"¹R5o-?È-'U?ïôëB"á4?@Áy@+·?V)zé{gS?@Áy@+·?ï÷È»|Ã?^ÅkÈèŸ?PoÄSJ?^ÅkÈèŸ?ï>¡UЗ?¤#ÿ'ñ(?˜+ÕEí(?¤#ÿ'ñ(?î֖(¯û?–'Äbgu§?¢–v)W?–'Äbgu§?ïRܤíEú?ˆ¸äSc}?•¤kbW@·?ˆ¸äSc}AGN3FGL J1015.0+4925@d±?Ýe¡@J[‰€Fâ=À7%cèä÷À:5›Jt?ì"$áûvó@э7`"j?ýU®€0'î¿ÚªðåÁ÷m¿ÚÔm®6è'¿ÜŽHõ¿ÙãÔåŽÔ]AGNbll@"W™™™™šPowerLaw1H 1013+498?ïþqw?"¯v¢ÀÞÜ?(î'6¸Ý>?"¯v¢ÀÞÜ?ïÝÓ6b+ˆ?w˜¨"eƒ?qd¿?w˜¨"eƒ?îäÌp'? ¸hY?¡³>7Fˆé? ¸hY?ï–%ktm:?p)s– ¥~?Šv¥"ä±p?p)s– ¥~?ïüB]j
Ø?=1H«J0"?=í"ǹ?=1H«J0"?ï-±Só? Z)Ÿ¿+,?šI՞óï¨? Z)Ÿ¿+,?îú–É}ƒ?œÂSÆ'vy? V"dÀ+Ñ?œÂSÆ'vy?îH8ËE?Ÿ´6g	?®Ë|roȶ?Ÿ´6g	AGN3FGL J1015.2-4512@qC$ÜY2@"ÊÊërªÀ9î"
>À;•¹Ù«¡Àð'äÄeJ@‰ý²rÙf@é4Â='¿áSó:¿à
sÒEí'<|T‡?×ރi½šAGNbcu@—ÛW>«6PowerLawPMN J1014-4508?ïóžJV?dЕ$ª…?XÃ×<dË?dЕ$ª…?ïÄ<8{®?‹µWë?}õaã=(?‹µWë?ïpޏlïí?‡è'ʈõ"?'ä.òfX?‡è'ʈõ"?ïÿÿîÑô>bô·30wS>aSkùp->bô·30wS?ïg9m	×?—6lòžLð?"Òdo"?—6lòžLð?îÎn‹V"?¶s~â¨#?£J–É?¶s~â¨#?îX&sËîo? žû£ú?ª}˜Æ°µ? žû£ú?ïÿù‡ÀÔ>ÚõßeC¦>Éá"m4kP>ÚõßeC¦AGN3FGL J1016.0+0513@mb€'،@GƒüõŠÀ8K¯é(À;)€,?çAÎüýÂ
@@–Ì_¿ƒ@õß_÷av¿á°à.m?¿å»WeÜA¤¿Ü÷¹èø¿ãw×èè>÷AGNfsrq@™¿—$tTPowerLawTXS 1013+054?ïÿµÀÚ2?²L¯öÙÉ?ðX‡³"?²L¯öÙÉ?ïÛzéÄî÷?ƒwŠŽVtø?rB‹¤Í?ƒwŠŽVtø?ïða"Éri?Yѹ»ãô?_=ºm-Ð?Yѹ»ãô?ïýç|Pˆ"?sIP¸?0Ä'"h?sIP¸?ïÿ´Ú,?v$:K>þþŒY|?v$:K?ïYüxê€?šSÿAÐ@0?"ÀpÛÐÄÖ?šSÿAÐ@0?ïìa.»v±?p_\Ñ!#F?cžÑMÿ¶?p_\Ñ!#F?ïû8÷´N?;
\,Šãà?C"¾?;
\,ŠãàAGN3FGL J1016.0-0635@o"ddIV@CÂb¿è¸¼À:A/)¹6îÀ;ÐìwŒÿ?é˜O·Î8@6§µ\™@Z]ÿ—¸?ŒóžGÔ*¿æ*[—ö¿íK£'è¿ïÿ°FP¾¬AGNbcu@ƒWë@öjUPowerLawNVSS J101626-063624?ïôq&*Y?`z7œØø?Vý m~ú?`z7œØø?íØÚ9qæ¢?§Ð™|f£?±9.4×o?§Ð™|f£?í¯ÜŸÂ? ¹û˜J
Ñ?²‡á!¢Ïê? ¹û˜J
Ñ?êÄV0¹0?žÞ
"?DŽî§=>?žÞ
"?ïõÞùlŠd?^Ô|?%å¯?TB
GçwT?^Ô|?%å¯?ᒕ®Ógœ?ÐSDt
û?ÜÚÔ¢Y0É?ÐSDt
û?íSÚ;[†ö?¤'r¸í?µa.$µÔÔ?¤'r¸í?ˍaEó3?«­å?駮¸Ã3?«­åMIXED3FGL J1016.1+5555@c'7¼]ê@I' ("tÀ9ÿÓ3[AÀ<Š7üÇ?'Ž»Á¢ý@×`Ô+:ì@3Úÿ•võ¿ä>"èÚÊf¿ç>y|1˜˜¿ãW{¥ÎíJ¿ïÿÍ&}±öAGNbcu@…+ƒþ\'ÑPowerLawTXS 1012+560?ïÿ=]Œ*Ï?*Mòi<fŸ?TIæ!=ï?*Mòi<fŸ?ïÜL—2a&?"•pÝë0?qÙ´Xaù?"•pÝë0?ï²è:š
e?{á©K'ù`?ƒEñVe§?{á©K'ù`?ïÇGî'U"?a"š·"nÃ?|\Îâyþ?a"š·"nÃ?ïþst°š×?7(ÿÛq?(ȸ‹P´É?7(ÿÛq?îí¨ÆCñ?«´E?ÅÕÇ?¡%sž[•ë?«´E?ÅÕÇ?Fàº?‰+ìáê?‰Õ®N°²Ó?‰+ìáê?íG[Cr›~?£BÐAï­?µÅ%äk$?£BÐAï­AGN3FGL J1016.3-5858@qÁUÿæՍ¿þMV¾|'À7s­uïpÀ9¢ì,
¥?û&…}'âž@¼œ®L9@GÔJDœ½¿á¡—Ú§¬¿àÒ¡'Ïe¿æB°ÊkQ:¿ìU}ÃOJ–PSRPSR@Ÿ¼£PLExpCutoffPSR J1016-5857?ckéö¼Õ?g‰²"2Î?ïìþ"÷̳?g‰²"2Î?©6~çóŒ?¼5ÍÔðÄ?îl˜·Á?¼5ÍÔðÄ?¿¹ýšÓ‰?©$±Né¨?ìÀL¥Žß?©$±Né¨?ƂÎò~? ž"Óë ?ê_LCz~ ? ž"Óë ?5'¥þ…@A?/pú"Ãä?ïý[$²x?/pú"Ãä?†ýp"οÒ?ŸÕ2ßÁÀ+?ï¤
=hÑ?ŸÕ2ßÁÀ+?¦–åä ?žgëWĐ}?îŸ6'Œ"Þ?žgëWĐ}?›{µÆ'?"›ç9¦
?ï$"QÂ$?"›ç9¦
PSR3FGL J1018.1+1904@k1  ôØ@Jýb¿è¸¼À9³e·ýäÀ;§'ûç2¿ìŽøjNAE@ؾoçÄu?ÿ¼Á¿}ƒä¿ç2lw*6"¿×ׂÍ2¿ãøãÊ¿²ïæéiÍAGNbll@¢|‰º^5?PowerLawNVSS J101808+190614?ïÿQƒD1w?
÷@tó–—?ϗqQø?
÷@tó–—?ï蕶ò+<?kNû†¸²4?gjI*±{ƒ?kNû†¸²4?ïê.]¶j?gˆÐá"à?eüш,Ž›?gˆÐá"à?ïÿÞl(ê|>æ{9UºÞ?>ðÉËÜÂfš>æ{9UºÞ??ïÿ'[óØ? v?$N?í¼[mEO? v?$N?ï0–¿äJÝ?±êÿ'†Ì?™í'ü—lx?±êÿ'†Ì?ïãXH&Æz?t‰(%—¢÷?l§·Õþ~?t‰(%—¢÷?ïý®àlY?2ÞnSö'ˆ?2‰¾Ïbv?2ÞnSö'ˆAGN3FGL J1018.3+3542@gŽï€Uûµ@L:. &{•À:,G"GÛÀ;ç¥b$¸F?â³Ôœ±d@äDó¤ýÑ@d'Ÿ¥!b¿åŠº3 žú¿çë}®ùÊ~¿åË©tX¿ïþq|ýAGNfsrq@‡÷ޓž®PowerLawB2 1015+35B?ïÿšµ"Œ?—Œ?	R¼d¸}~?—Œ?ï×Ħr?X~Ø^a›?tý;‰~Ó?X~Ø^a›?ïÁ]Y'/­?dLpÖ]Ãu?QS6QÀ?dLpÖ]Ãu?ïdËÃÁ?m¬ñ[ë—Í?¦ý	ŸsË?m¬ñ[ë—Í?ïÿË´Ñ9>ûÆkrÁM>ú&wQÀð>ûÆkrÁM?îøK¤°?¢w%¿ùÐ? {Nb¶?¢w%¿ùÐ?ïÖÄßåÑ?tœâ)ýi?tôªÚŠ?tœâ)ýi?쌨šh?§oÕ ¿yc?¿×š»,¼?§oÕ ¿ycAGN3FGL J1018.4-3119@pÆp_®¼A@5!@ÂgïÀ9€÷¹à`þÀ;ëg†ù?ðzÁDXt‹@¤æÛkÌ@D…ßÓdÁ¿Ú̆žó©8¿èsá".c¿ëT³Ý¬\Ú¿ïôf¶1C´AGNfsrq@ƒÐŸ¾vÉPowerLawPKS 1016-311?ï®{¾gYV?‰^»V•©?"aeÑ´Ÿ?‰^»V•©?ëo¾n4ø?¸æ?ÃL?ÂAîG, ?¸æ?ÃL?îìÏ1ð­?"pƒÃø?¡8,x.?"pƒÃø?èqàÜ4"þ?›•þY""?Î8|-ì?›•þY""?îí¨û%??©<H©¾µ?¡/¥s½H?©<H©¾µ?Ø®_¥h@?Ï
 ¾*1?ã¨Ð-Kßõ?Ï
 ¾*1?éÐÔ`aa?µ?§Å @y?ȼ®~z{¿?µ?§Å @y?ÉÈé›(?¢¼­uª/?éÅ¾™5ú?¢¼­uª/MIXED3FGL J1018.5+0530@m–/IŒ;@GÙUÿæՍÀ9V‰µöÇrÀ;S 'àð?ñêâצ°@l"6Ûß@ΓÏ,?îMKMV9¿ã ó粛¿èk¡—ÐýÅ¿ä}å-AGNfsrq@"?1&éxÕPowerLawTXS 1015+057?ï:ÂfÊíØ?Ÿ"&ZT+É?˜§³?
?Ÿ"&ZT+É?î5'©Î?¯
4é á?¬§,©|?¯
4é á?î(·Žø?žU™7ìM?­t‡¤ì?žU™7ìM?ë°ÒX°xâ?¡à¼äáç?Á<¶>y?¡à¼äáç?ë'Ù\?â=ü~¯ø?ý÷ðšì?â=ü~¯ø?ç# ¯4x?ȯÒêš#?Ѹ¾¡Õ—?ȯÒêš#?éß>ir4?±S+«g?ÉȃZ7.?±S+«g?ÞU"/¾Î?¾àíÚÓ9'?àþÕ=è ™?¾àíÚÓ9'MIXED3FGL J1018.8+5913@bî´ßݵ@HJa€M˜9À:ilØ{À<&¿è+οñ~:Ãu`@ȈD‡™@¹,?Î÷õ¿å›Z—ŽI¿âYl"=·¿Þ^…Ø'Ê¿Øó†FÍç!AGNbll@ Ÿb'@·€PowerLawTXS 1015+594?ïÿ³õ:?$'ë£àd?)‡=7Åj?$'ë£àd?ïâB'=[?'f¼RÑ; ?m½mð´þ?'f¼RÑ; ?ïà"4*æ?rÞ<IÓüË?o{ê®øb?rÞ<IÓüË?ïÿÉ!Ø©
>ð+TFBjÝ>ûo">ð+TFBjÝ?ïü§
©"??¬Š-ªN;?:ǔL4ß??¬Š-ªN;?­¹Gp?'¬³"'?Œ\"•¿÷?'¬³"'?ï·õòàÞ?…ÇU±»¸ù?'=Œ6Ċ?…ÇU±»¸ù?ïüŠ84`?8È‹?;¯×±ÿŠ ?8È‹AGN3FGL J1018.9-5856@qŞ 3玿û
¬RÐÝÀ6ϽBNÀ9'¤g¡Ð@lá//m@
ô܄¥Á›@òƒë‡x¿Ù£ôüÁ²¿å¯íÎ¥!¿ç¶%÷
ø¿íTš\78OTHERHMB@•Û"Ðå`LogParabola1FGL J1018.6-5856?6zæËPÄ?@ƒÊiž?ïý0£žv?@ƒÊiž?¡ÐÇÀ3çW?¾ùˆRۀU?îâó"
ú?¾ùˆRۀU?±Ê:xTª?¦¢ÕЩµ?íƸ±6ï*?¦¢ÕЩµ?>#¥Œ0†¾?-‹·6|Á<?ïü;‹'Ð?-‹·6|Á<?DoûýDr?Dl©¨.…?ïúäGÓ?Dl©¨.…?ˆkôe…$s?ªé¹ €?ïžP.…hN?ªé¹ €?¤@¥7rã?¤‰ôÑ&7?î»ÿ…ºGB?¤‰ôÑ&7?o醜D<?FãQ×{$?ïÿt€õ!Ä?FãQ×{$PSR3FGL J1020.0-5749@q½ž 3玿åeSßÙ¢|À7¼ií£ùÀ9Ñޜ)¦?ñØ$ ñ')@Ý‰ˆk@¦nmXž¿—?¨®×»¶¿ç¶®t¿g¿ä1yðºp\¿éc`!¢½PSRPSR@¤ïiDg8PowerLawPSR J1019-5749?Û¥íïvà?Ѽgò$?â-	Dû?Ѽgò$?ì¥töî?º·5÷2Ñä?ºÔXOø'?º·5÷2Ñä?ß!!+/?µÀš­ssÉ?àovojhv?µÀš­ssÉ?ëâ5×Òö?"	nU"R?Àw)ˆ ´&?"	nU"R?ˉ«Øéï%?ÉÓVÐW'?é•	ń7?ÉÓVÐW'?ÙDQ­`?ÇÊHo°?ã~]×)O¸?ÇÊHo°?ÚxÈt‰¥í?º5ÉiÚ¨ò?âÛŻ-
?º5ÉiÚ¨ò?áÂ÷ Í^?°ž)hŸ?Üzá¾eE?°ž)hŸMIXED3FGL J1020.0+6323@bK^?»×²@G"_£Ô†À:+)­xs¯À<ìÀˆì?ëó0Ùç'v@
c~Ì
à@Kø`îW?î×·¿D=¿ä^häq¿êY4ð¿ä|#È9ȬAGNbll@'üT`ªdÃPowerLawGB6 J1019+6319?ïÑÚ6S	y?ˆˆ¾™2M?w䷎Çå?ˆˆ¾™2M?íEZ¦×?¸ZS©7€Ò?·Õ0—I?¸ZS©7€Ò?î¡Ñ8›?—ìT-î?¥âï®6$M?—ìT-î?éñˆ ¨õ‹?¨YƂÌG?È9ß}\)Õ?¨YƂÌG?îæ%鞔«?§†9ÇJL—?¡¡fòœM?§†9ÇJL—?âÎ[îm?͕pïE6…?ÛÜcH#Û'?͕pïE6…?êR‡‹=úü?±æMÝg?ƵáÓ?±æMÝg?Іô:úÒÅ?½æ QTm?缅ₖž?½æ QTmMIXED3FGL J1021.8+8023@`@Iÿ'ò¶@AKg€AÙ¿À9é-¡"ú×À;ù/À·ë"?êÀû1Ühn@_ih¤Y;@!@—tѿ吒fõW…¿ç—nµÚ¿ß9,"ç
ï¿ïÿ±žs.AGNbcu@'6E¡ÊÁPowerLawNVSS J102201+802350?ïz×_€v»?j»9ñK.?¥Ð`‡?j»9ñK.?â¸ìò à¥?ËõꝘ+Û?ڎ&¾>·?ËõꝘ+Û?ìàv¤ïZŽ?¦V я\Ý?¸üJÚ<ù?¦V я\Ý?ãlDN?¬Í]PÊ1?Ù'wcõÙó?¬Í]PÊ1?îmŠB}m?±dg)¥ƒ?©#×_GÅ.?±dg)¥ƒ?ÈG¡t"aN?Ëögۆy?éî¢Þç¬?Ëögۆy?æºÕ³-Î?¼6,¬
?ҊT™×¤d?¼6,¬
?¼}'Õ*ó?¦ëdÖX¼?ìpO°Z¢?¦ëdÖX¼MIXED3FGL J1022.3-4234@q<‡¿çáü@(š"ÿ%ÀÀ:Au}Zž²À;¦ÝÉtR¸¿æ¼ ÜGØË@Q®Ÿð¡@° M¼¿é‡wÏU¤]¿ãÓ?
_ˆ¿ãn,\€¿í¬"Ç
Ò'AGNbcu@•Òÿ¼PowerLawPMN J1022-4232?ï¨ûãL?'i­ÃE-<?…ù}Çædø?'i­ÃE-<?ïƑµR:h?ŒJɾ)ºÇ?|·%@5`?ŒJɾ)ºÇ?îpªsËB£?—TÎTNp?¨õXÄ'¼Ñ?—TÎTNp?ïù	*v ?8:ø?â§K?K‡Ú»†3?8:ø?â§K?ïzxKì·?ŽÁWuy?°ö"5—,?ŽÁWuy?îß^¸z¸á?°ópVj ?¢
täÕî?°ópVj ?ì÷¦·‡?­ÑP"Ã?¿{€BÊCÊ?­ÑP"Ã?ïn áPVH?‡¸'œ/?'+ã҅šõ?‡¸'œ/AGN3FGL J1022.8-0113@n¨Äê@F0³ß•ý-À9#a.AÀ;p×%+3?èp/¡òóA@-hì'°ô?ýþjaÐp¿æ—ÿW?ˆ]Úü^ݿ׈ô'Q¿äö­Þl~ÑAGNbll@¦\)PowerLawRX J1022.7-0112?ï,¯9O=;?Âþò
ùèº?šj́R¦?Âþò
ùèº?ï…×^1tÓ?‰þc&zo?ŽŠ(}ñŸ?‰þc&zo?ïÃxHÍ4?€3ÒÄÎE²?~CۚőŽ?€3ÒÄÎE²?íÂπäÊx?Šö®"õ½S?±éƒøk¸À?Šö®"õ½S?ïͳ>RÃi?Ì@E…á?y&`»!kÅ?Ì@E…á?ë4t}o0S?¾âGµü?Ã..
C>³?¾âGµü?ïo%ÁtmÕ?ŽöêhÐ4?'GÓ*b?ŽöêhÐ4?ä‡Äᵬ?²npÅË?ÖñÎv<"¨?²npÅËAGN3FGL J1023.1+3952@f—|€"Þ@LlØà†8À9ßZ"‹ECÀ;䇀'a—?âk¬D}C´@~P¿54•@ÎÇà(õ¿å£€¢Ÿ5¿ëËåŠø†¿ïþ¥l-:?ïȧèMAGNfsrq@|ìZîcŠPowerLaw4C +40.25?ïÿÚVUÕ¨>üõL)ºIË>òÔךÎ
•>üõL)ºIË?ïæ÷r½.?|#ÈÊCl?iÁiÚI?|#ÈÊCl?ïӀ՟ю?kz½0´•?v?•NSȜ?kz½0´•?ïÿ³aõF?¿"ûÊ?'jâ?¿"ûÊ?ïÿÂÆ
ÀÞ?"dmŠì>þœíÒÓÉ?"dmŠì?ïmS	è65?¡ÊÚr?'UžÁAkj?¡ÊÚr?ï'íÀ.Ñ?"©Þ‹;2?‹D
) ?"©Þ‹;2?ïú'Ëï¥?[èÌ[#?GcW?[èÌ[#AGN3FGL J1023.1-5745@qÂÉ?¯Bx¿Ù2ÿÔ™À6¢0'åøÀ9…{2¦Ez@Ïnc¨@܄¥Á›?ýp؍JUå?ìõÒL–S¿â#N+\$C¿çæ+¿1¿Ò¿ì:Õ_â¥PSRPSR@£æÿ—$tPLExpCutoffLAT PSR J1023-5746?4Gßş•€?2~€?ïýwíud?2~€?¤™tA·q?ÂÈgjûÕ?î¶h»ïô‰?ÂÈgjûÕ?€ýs#\RF?ˆœ…Uk¡¢?ï¼
3ymï?ˆœ…Uk¡¢?sm
Ô¼ËÇ?aDd™Š#?ïÙ%äHÇù?aDd™Š#?4E"kÐ?-¥ +ÝãF?ïýw\'âÉ?-¥ +ÝãF?€~)5äT‡?œÉÝÌQçN?ï¾[$O&?œÉÝÌQçN?tc/Hn¹?j,ŸñсÑ?ï×9¡¦N?j,ŸñсÑ?QBÂ^rÉ?JôTÓhÏ?ï÷^ôW*^?JôTÓhÏPSR3FGL J1023.7+3000@hÞeÀ¹™@LËèÀHZÀ:‰'³ò
tÀ;Ü&¯—1à¿ÉæM:<ß@
cäz=ˆÍ?ûîþ?áll¿è㎘';4¿å‰}AR¿ÀYå4ÞÀ&¿Ò§¶|d'AGNbll@¶¶R-VPowerLawRX J1023.6+3001?ïÿ{ÎáÁ?Šç‡…%6?† ÎJ1Ñ?Šç‡…%6?ïۓ›ö¯?†Ï&K÷­Õ?r62éäÀ?†Ï&K÷­Õ?ïèÑH:4?g®[õ€"u?g.·™Ðô>?g®[õ€"u?ïý@ê^Œ?$¨}pΐû?7Íú4xº?$¨}pΐû?ïÿ*±É*?FyP¨²?©ÌÈ>­?FyP¨²?ïa—u?¤þLAd2á?"Ý-'9?¤þLAd2á?ïèÄCޞ~?gÌ­€_?g;¼£B?gÌ­€_?ïæ²–`L?e`aN0?iMâw^$[?e`aN0AGN3FGL J1023.9-4335@qIo@_k @':¢?ZˆãÀ8Ȕ¤gRõÀ;ìþ›{ò?Åëô
3î@¶b®ËÚß?üŸ[à{€T?Ülä¸Y¿ß]"–Ž]¿ÝZYOº¿µZeÞùlŠAGNbll@¬'l"h	ÕPowerLawRX J1023.9-4336?ïù\J·;õ?AJw$&3q?JŽÔŽ¡Ì?AJw$&3q?ïºÉ¡Ó
?'®¹p·h±?M¹^Âkh?'®¹p·h±?Zû)?}.4Nnր?€ÑA1ÀÅÂ?}.4Nnր?ïõ}Hç5À?@÷Vg°ˆ\?Un<"@$?@÷Vg°ˆ\?ïè'iéA'?b6˜¿ëB"?gm–/{ž?b6˜¿ëB"?´ðY'?³©M[œl?¤6Ô®f±ð?³©M[œl?ïvòÍèU¿?'2n܆?'!¦IԀ
?'2n܆?ï«ÿGœ?{™]‡æ+?…9»×iÛ?{™]‡æ+AGN3FGL J1024.1-3232@pãrà\̊@4Ðï 6kÍÀ8¡ÃPLH®À;uÝæЄ?ó•xÕ©À-@¦mV½@¦L A©n¿äŠ«Áå=¿çž9='A§¿çŒ¶@],¿æ::×þjeAGNfsrq@'ÚÚ¬1PowerLawPKS 1021-323?ïÿ<3í?Y2ó{P?yšNvê
?Y2ó{P?ïÃ[b¸m+?Júߋ""?~RN†<Æã?Júߋ""?ᄂñÅd?yC×D?€VÜԌâ?yC×D?ïÝFçüî?Q¦Ö
©í?q\Œ—®U?Q¦Ö
©í?ïþ‰-ؐ?'®;cØ}?'m-ŠnŒ?'®;cØ}?îÅü6zn?µ8¡üdv?£ <—}8$?µ8¡üdv?ï£^¿S ?…—gÑz¥p?‡(P}(?…—gÑz¥p?ï†XJUý?~ºßf濖?ŽiígH¤å?~ºßf濖AGN3FGL J1024.6-0718@ouÛߏG0@DB+ ?:¨À:Z÷xr¥À<J§Å¬G?ù	ùé-@5ò1
d?絫ºrF¿íqTsD‡?êÜiÔ¿èABah>¿ïÿ­µ/w<PSRPSR@ 7
quŽPLExpCutoffPSR J1024-0719?°u¦þLšº?À"l¤Ì†4?íñK (®9?À"l¤Ì†4?ξÐ9˜l?ÏG°å:­?èPKüq™å?ÏG°å:­?Û+qdé†
?ºRs¸<?âjGM‹<ù?ºRs¸<?Éîo²ž?²,/Ï·žù?é"dXü?²,/Ï·žù?ÅÁˆˆ7?ҔVÂ7%9?ꏝúà2?ҔVÂ7%9?µüä&¤'C?ãŠÅQ"ƒ?í@c{2h?ãŠÅQ"ƒ?Ôÿøü´$?¸&06Ô}?åñ€¥î?¸&06Ô}?'ªµƒ–?…¯5S?ïwBª}C?…¯5SPSR3FGL J1024.8+0105@ngààëgÃ@G$:`NqÀ9Ýë˕•(À;¹ÀI0Ëz?ïcV†Ê_	@
ª£¶~â@d±€9"¿à'…gÏ¿èåÍ-}¿ìK9ðø·H¿ãöÉï!áAGNbcu@'@¢‡PowerLawPMN J1024+0056?ïæ'jŽOu?p»²q»?iؕ<£‡?p»²q»?ëÝú"Îë?º1ë:ȱ?À‹ätÄV?º1ë:ȱ?îíšÏ'<?"ÙaLúnA?¡.¦QP<?"ÙaLúnA?édñÂX2O?¥ÍÝ©oÏ?Êl8öŸ6Å?¥ÍÝ©oÏ?îᙴ¶Dd?¨3^–«?¡æd¶S‡¾?¨3^–«?ÖZhSÿâ?Ϟ³3ôy9?äÒËÖq€?Ϟ³3ôy9?ëhÇ!š?°G­o¢-?Â\ã»{Á—?°G­o¢-?ǔÅhÝî?µ¦#[3^?êüΥȅ?µ¦#[3^MIXED3FGL J1025.1+2333@jZe>‰©@LoüõŠÀ:"ÜޓÀ;ã÷YhQ"¿ºþãA@ÉAÂUP@™ †¿åÞ¡ï\!r¿ìqz@¸Ø¿­xÕ~]d¿ì{¡ß8_BAGNbll@ƒe¯·éPowerLawMG2 J102456+2332?ïúèbп?AÚÑqÁ>?D^xN"Já?AÚÑqÁ>?ïÜXü˜2?€¿ðÞ€'?qӁÙFËF?€¿ðÞ€'?ïL‰WÏl1?‹ö0'QÎ??–nÕÊGä?‹ö0'QÎ??ïàðÇË(?Z´°Bá<?oüd/Ø?Z´°Bá<?ïúÇj|?IÿâµÍ?Eˆáô4€?IÿâµÍ?ïïz¼£?ªá}ˆþ?œ¢îð"?ªá}ˆþ?ï[K'5?"	›Hì?"–›$˜—?"	›Hì?ï†)OY¯?—á|Ý W?Ÿ/:Ï5'?—á|Ý WAGN3FGL J1026.4-8542@r®€{»bÀ7¥pà<ìÀ9Q½‹ç)À;}«Âßä¿åtªÊ¢Ò@
×á°ß†c@\à*͉¿å€4$Â#ž¿âB÷ÑÕ¿Ù[$_AY¿Ý»‰-±éAGNbll@¡]lcñA PowerLawPKS 1029-85?ïø\?›÷B?K†	Æq?NA…'Y?K†	Æq?ï̞¸ÿ?‡˜ìµ`?y°¹(ÿ X?‡˜ìµ`?ïÃXƒ'£?}a#%ßæ˜?~S±2ˆ'Œ?}a#%ßæ˜?ïü§4Ú¼?+Š}ðþ?:ÆZ%T'?+Š}ðþ?ïñþˆËZ?^B
B?]Ôg¸œÑ?^B
B?î¨|±ŠØ?µrP¹É?¥x4êÏ^{?µrP¹É?ï˜ ‡¬S¨?Š'­zoÞ?‰÷ÞZ²?Š'­zoÞ?ïÐi3G;?ożÏћ?wË)V)?ożÏћAGN3FGL J1026.5+7423@`ØÑ Äe@Cœ¦ßÓ9ÎÀ:Nd!À;ˆºô]4Ž¿Ý·P‡4šÅ@´A€}é»@•= t.¿èΙ«7¿ìó?ôüZž¿Ä
‰d‡¿çÍRh؆"AGNbcu@‹·A½¥PowerLawGB6 J1027+7428?ïÿ‹5¨®_?UؤšÛ?
2‰ak¹?UؤšÛ?ïßØ1§9b?|u#Þ£"?pç-Ã'?|u#Þ£"?ï旂×Ïú?VB¥
5ˆ¦?ih}YªeÏ?VB¥
5ˆ¦?ïû¯ÈÒc²?-¦"(ì]a?A@ܼ}Tâ?-¦"(ì]a?ïÿ"8{Á?íÀå?1Ð4~êÞ?íÀå?ï6@ZÛe?§¥Si½ ?™=ùËýR?§¥Si½ ?ïÏÉ)æ>Ÿ?wx×óž?xjû¸•?wx×óž?ïÞO›ô'º?hvæl(BÏ?pØ2¶£@?hvæl(BÏAGN3FGL J1026.9-1750@pNÔ@(äü@@\ßÔçNÀ8Ÿ–/ÍËÀ;,WvßZ?߶ÞÓ#lÛ@}ÙõI?þ·ÖÁañ¿à]ý<½[ҿ܀¯õó¾¿Ý!+‰E¹s¿Ùo¸ÕOAGNbll@ž]Ϫ͞"PowerLaw1RXS J102658.5-174905?ïÿœF¶âo?u2Æ~?îFmw¬?u2Æ~?ïÞ#¹§?y™3'S¯?pît«»<§?y™3'S¯?ïå	 )?n,^û´{þ?jöߺ)?n,^û´{þ?ïûï–V?#'›S&%?@C²«v¿ú?#'›S&%?ïÿ7³þþ?"õ†;ö™?V·"á?"õ†;ö™?ï:RFýH?ª[ì/«£¹?˜µ·Ÿ.W?ª[ì/«£¹?ïæõÔ`ž?rªdוߘ?iî
V:ŠC?rªdוߘ?ïð0?QE—kÆgx?_å^c?š?QE—kÆgxAGN3FGL J1027.0+0609@m·±~þá@Hç3çüÔÀ:\øÍØÀ;ÓÐJ/Îû?×°ý˜G@¤H"Xšv@¿¯ß/j¿ïòýý¶?ÍHਿ犋¸k¨¿Ðqþ4£Ë¢AGNbll@¤ˆ×
=p¤PowerLawNVSS J102703+060934?ïüºç$Åe?>|°×4ú?:(ȑ¢Öä?>|°×4ú?ïÕ'©‰ž?†vXɤ~?ul+*²Òl?†vXɤ~?ﺩà^D?w#tíÉaÕ?U‡ý€?w#tíÉaÕ?ïÔZt¸7?a(sõ"«?uÒŵÛ\p?a(sõ"«?ïé)³Ç\?i	lá?fÖLh¾y[?i	lá?îÚìÍÉ!?­—A»ç@N?¢Q3%%¼C?­—A»ç@N?ï,ë­&ƒ?"êV!T "?šbŠWÀú?"êV!T "?íµ]uãM?¦ ñ=úŸ?²US
?¦ ñ=úŸAGN3FGL J1027.7+6316@b6@ Ç@G€8_ÂÞ7À:s­]èÀ<)Ó8 Ù¿Ü­öaµkv@…¤ƒWÛ?ÿïkˆ±j¿ë¹²œR¿ØØ>ÚJ'°¿Õس#È ¿äÑ©u¯¯†AGNbll@¦~o\(õÃPowerLawRX J1027.4+6317?ïý{¢»?@ã")C?4"ð'C:Ú?@ã")C?ïÙõ)bO?†…@/ë·?skW)?†…@/ë·?ïÛq¿¤´ï?f…}š—ì?rG $ P?f…}š—ì?ïí¤iè?NÝ<lv`?b[ám¼È¨?NÝ<lv`?ïìR–"›?j"m>ؒ?cé­ e$m?j"m>ؒ?îéäö"?²<}Á™4f?¡g®
QÙ?²<}Á™4f?﯋‰ò˜Ê?ƒ"Œ"…?"ƒ×b?ƒ"Œ"…?îÒ¤<,Mˆ?™þy›Œí?¢Õ¼8車?™þy›ŒíAGN3FGL J1028.0+1829@k}ì_9K{@Kýfàé´À:_—+*P6À;ìRb£cG¿ù÷aüt	@Ǚ³oق@ä]_šÊ¿Öž?ý'3¿è;h³Ÿ_¿ßåå¼þy¿ÕÚÊPñŠAGNbcu@—ß·€4mÆPowerLawGB6 J1027+1831?ïÿP¹ð•ï?E)*|¥R?èÃØ~?E)*|¥R?ïâÐñÁñ?ƒJĆA¢?mú/8Ù6§?ƒJĆA¢?ïÕC¿P?uâpþ½Ü)?u^ i#|~?uâpþ½Ü)?ïÿôˆcÍk>Ì΋ƒþ+³>ÖïUŸx×L>Ì΋ƒþ+³?ïþΐ=?&ét;j@?#)jÍå?&ét;j@?ïaÖwyì?§v'Á¥w)?"Å1L†?§v'Á¥w)?殮ÂXó?ˆËoôgm
?†VcËa?ˆËoôgm
?ïþøØ]=?"ÅÎ÷&÷? r|î
%ë?"ÅÎ÷&÷AGN3FGL J1028.4-5819@qÑÆø¿ßµÿÿ˜ìÀ6ØSéŒ À9Ï´ÂêÌ@yuòËd@1<¸íó@®†‡C*Í¿É#»j"‹|¿á̈&œ'¿åé7ðS²¿ëÂθŸOPSRPSR@•'<ÓZ…ˆPLExpCutoffPSR J1028-5819?sCöù"Ä?†šŸœö—ã?ïÙxÿñ{?†šŸœö—ã?¢ÇD ç[?ÁŽ˜ùO{'?îӋ½ãÐÊ?ÁŽ˜ùO{'?¤BõñNÛ\? ®¡vYcú?î»Ð ÁÖú? ®¡vYcú?^€Y¯`?NX¡Í?ïð¿Ó¢˜?NX¡Í?^à&ïI£´?¸tëÐû?ïðì`¶?¸tëÐû?Jé@'?®GdçŒöÜ?ԑùM?®GdçŒöÜ?˜('!,ö?¢Ìv`F¡?ï>¿ª>i?¢Ìv`F¡?>Çr"%]?<üÁ¯È9?ïü'€Ÿ¼?<üÁ¯È9PSR3FGL J1028.5-0235@oN ‰ãC@FD!?ë¨ZÀ:^ÖÒ	L°À;՞¢ŸÓ¿Ü=ȋR6·@½;¾	;@9Nª¿àÛµ7QGh¿çü4Œ'7†¿áðzŸß¿çp¹Ô«*AGNfsrq@-‡_oÒ PowerLawPMN J1028-0237?ïÿê»"F>åê'‰ê>åDæ9›Îg>åê'‰ê?ïÞëæB"¥?}ý>W	?pŠô³-X?}ý>W	?ïëð¡ñµm?pþe]iH?d]õc?pþe]iH?ïþ¶\{‰—?ˆzz¾S?$š<t @¼?ˆzz¾S?ïÿ肂H<>ìèvɳ€Ì>ç}¤íÞM>ìèvɳ€Ì?ï@,ºëpH?¨æÏF=–?—úh§¹`í?¨æÏF=–?ïÏx¢—ÞÈ?ƒ0ûþ—*?xC®Î-£¾?ƒ0ûþ—*?ïò÷5x:?Pk㔛?Z•o6›R?Pk㔛AGN3FGL J1030.4-2030@pz-••@?eþßnÀ9¤ºB†MÀ;~o09ƒ¯¿µ*ÍóŽ8°@´ìL™á"?þ;bŸ1‰¿ã
]Nd¼î¿àÕAêáÇ¿Î?©˜5Á¿àkÎZXAGNbcu@§,ÅãS÷ÏPowerLawNVSS J103040-203032?ïþó¦ˆóã?SÿÌ	,z? ř孆;?SÿÌ	,z?ïÜô+zF?w
ÂïQÿ¡?q…êFü"ô?w
ÂïQÿ¡?ïíPE<Ë
?[<T"+ö'?b¯º›Y{´?[<T"+ö'?ï÷Ò-%¬?6‰õXÒj?P[¥®×ï˜?6‰õXÒj?ïýo‰û–å?2ƒq³*H?4ƒ²
^D?2ƒq³*H?ïH-¸—X?¬Àbƒj_?VúCÅ«?¬Àbƒj_?ïè¯söqâ?nVSÈ?gPŒ.©æ?nVSÈ?ïÄ(1ˆŸ]?pPRî"k?}ëçPýåœ?pPRî"kAGN3FGL J1031.2+5053@d.%¿­@K7èÀHZÀ94
ƒvA¦À;UÊÆbP¿ò–i¹W$@áë#$j?ûHŠàï§?²ïâ{ŠºÚ¿âÝoFVH¿ÒñŽÈá¿Ífl_hŠAGNbll@¬'Ý}¿H€PowerLaw1ES 1028+511?ïûÕ
—·?8sË©"?@«ÌéÑ»?8sË©"?ïè4TE|Œ?tFnú3¸?gË«ëýÓÏ?tFnú3¸?ïɘˆÞœ"?vFÊrJç?{3»oŠ?vFÊrJç?ïÿȘhIÉ>ñ«uº•µ>û³¶9V¤>ñ«uº•µ?ïùH0ÎÝ|?GÛυL?Jß<ì«æò?GÛυL?ïfx
Žài?¢:Ñ͒šw?"0þ¬l$Ù?¢:Ñ͒šw?ï»àËÖò?'fOP.ps?ßý<€?'fOP.ps?ïý>ß䬒?5eŒ¦T%ß?6	Œ/?5eŒ¦T%ßAGN3FGL J1031.6+6021@b"àç6@H›¿çáüÀ95?VW$ªÀ;UøZ?Ç% þä@	1í]ç@	?n)ÿ¿è˜ùX›øo¿çpØæi3©¿ÞµÕ
|Ú
¿í/ö‡,AGNfsrq@ŒÞ–¡aä÷PowerLawTXS 1028+605?ïýµÄ-Ó?/ýdð¦jÈ?2QÜÀOÔ?/ýdð¦jÈ?ïãßͺL?~ÏGÌ(T?l án¾ÓQ?~ÏGÌ(T?ïIÖ_—ý?Œ¶wžÏ?–Å4!üœL?Œ¶wžÏ?ïöÈG'?7«Æ‡ô9?Roó'‰lµ?7«Æ‡ô9?ïþϘ?&ȪØ·?#€‡ìXú?&ȪØ·?ïC«ÑT›ä?§½—‡'þA?—Š…Ø܇?§½—‡'þA?ïFúD!¤?'èÍ$Š?— ·tdŖ?'èÍ$Š?ïÎs2,³?nÍυQ¡¨?xÆfòùjc?nÍυQ¡¨AGN3FGL J1032.5+6623@a»/ÀL‹Ê@F¦>ÿðÈÀ:ìÕy(
À<MiŠÞô¿Çæ²üìû@A'Ž³6¤@2o¿¨Í¿êÚԊ¹àj¿ÛâîwAý¿åþR—¿ÝÀÖw¤	AGNbll@ž'nzáHPowerLawSDSS J103239.06+662323.2?ïå|³§.O?ƒÍ•Å¹Ó?jƒL˜
€"?ƒÍ•Å¹Ó?ïÜ¡Y_~?…>¾r:0Þ?q¯Sp¨ë?…>¾r:0Þ?îFqBQM?¡ùšà;u"?«˜ë֟«Ï?¡ùšà;u"?ïùl1Îс?6a69
?JO8ސ¤¦?6a69
?ï ƒÛÂ3?'ys'wº¸?‡ûßî«1?'ys'wº¸?ï,wYu3«?ª±òOð¤?šqÏ¡¼ž?ª±òOð¤?î*Å«<я?¡¶"ׂÂÄ?­S¥Mêµ?¡¶"ׂÂÄ?òÁ†¦?ƒ6Jfkôå?ŒWOžVu?ƒ6JfkôåAGN3FGL J1032.7+3735@g
Âß
A1@M‡9á£À9A§~^ª°À;ʒ~e'¿í!ìè0"@Rk~SB@™÷?':¿äìðgAéÁ¿å*<éâ©¥¿âX<'ß©/¿ä²T²ERAGNbll@ˆOr f<uPowerLawB3 1029+378?ïýY9W?3µ@Ûl—?7߇-ÈÐE?3µ@Ûl—?ïãCÏÁ&"?€Ú;³|õ?l¼0 O?€Ú;³|õ?ï¿ç˜næ?-Ù¹Ž9?€Ü·[å?-Ù¹Ž9?ïû&Š›
?7˜¤ÑEoÌ?Cg'âhx±?7˜¤ÑEoÌ?ï÷¤¶G)?N+ÌJ)?P¶"ÔÎmö?N+ÌJ)?ïLÏ(ǟf?¨`…ÛB?–fà,Û=?¨`…ÛB?ï;¥2²d?'Ú~] fŠ?˜‹Y­ïz?'Ú~] fŠ?ïzí'úߞ?ŠõýNži?¢ZùÄÔ:?ŠõýNžiAGN3FGL J1033.2+4116@f+zß.Ï @M2R¿ÀtÐÀ8áî¯u£ñÀ;·uª§?ÖLž?Vé,@à Áìt@'Ð pË¿ßa£½‰ä¿çB‡ÜOC¿à<%ÿ²Áø¿ì#ٍiNgAGNfsrq@†ÒÄ2ÊW¨PowerLawS4 1030+41?ï´Ø%ŠAý?¶l׶/ç?'Éö¢>ôÔ?¶l׶/ç?ïÞóX°Mï?x"Ö\\¾?p†S'ÛˆÊ?x"Ö\\¾?ïsiiP%²?ˆR¼‰žæ?''ÒÙjå³?ˆR¼‰žæ?ïϜŠ\1Q?^%­QoþÒ?x1ºÎw»±?^%­QoþÒ?ïý//Üú?8§ÓŽrø?6†ƒ_xÕ?8§ÓŽrø?ï%²ƞ"?¨¥W}†?›I½#¼'¤?¨¥W}†?ïb0ÕJ?= a'$?"¿Ž¿?= a'$?><%Ë?–¦D°…¯²?¦µ,…ÕQ?–¦D°…¯²AGN3FGL J1033.8+6051@bxæÿ}ú@HŒö@c^À7Ç9k[˜­À:Ñ«ì'tº?úy4I]Áý@æ~ZÎؖ?ÿļ'ÂåÿÙ蘙®+;¿âÛÆT¸"¿ä qFŒ¿èjó®AGNFSRQ@Û ¥&–LogParabolaS4 1030+61?ïûm'[õ°?CE,˜}N?BKb#Ûõ¡?CE,˜}N?ïãþ±e,?~1"ÝUN?lNj¹_Ç?~1"ÝUN?îsŽqÄá? H¦Ôä ?¨ÇOüø? H¦Ôä ?ïþ2"˜½?G³nâA
?,ÞûX¤	-?G³nâA
?ïñŸ"D£?^8âÈçW?]ÄÁk¿É‰?^8âÈçW?ïWܬ­ŒZ?©3k|ж?•jm¾Ë?©3k|ж?î<¿›XX?£†Ž3Ï?¯œ4H~?£†Ž3Ï?ïþlÜĈþ?(ÔpϏ–\?)26©³÷\?(ÔpϏ–\AGN3FGL J1035.2+5545@c?ʞõ#-@J/xßå®EÀ:*ôœõn­À;ñ<¼HñÀK|7³ög@Þ/â+Y@‹õ €"Ž¿èe~Ñ[¿¿éöíO×·?¿é«k¿îøË1}bAGNbcu@v[^ FÇePowerLawGB6 J1035+5542?ïûýv=–?>oO˜ÂwÀ?@ÝsD}ô?>oO˜ÂwÀ?ïä#›e¡š?€œ"ÿè·F?kÜdcd¥Ý?€œ"ÿè·F?ï;:ÏÅâ?ˆ<0ç¬â?Œ±1O~#?ˆ<0ç¬â?ïÿýúþI®>°`C´œT*>°&Îå/0ß>°`C´œT*?ïþžÿ4(&?,S¡-zc?&	qÜ8?,S¡-zc?ï\AƒûD&?«ÞAñ°ë?"wςOI@?«ÞAñ°ë?ï¶#ÙV¦ˆ?ŠPî0|ü?'w	³EY×?ŠPî0|ü?ïÿˆO©ê?H ŽMc}?
øhMó†&?H ŽMc}AGN3FGL J1036.0-8317@r®½_ÜßjÀ5O_¹£ûÀ9àG­=»LÀ;®ygÊêt?ê÷6õé@
ùpò[|¨@¤H©hš¿«_QÒ¹(‰¿æL!·hj*¿æö}‡-Ì¿ïÿ-zYPSRpsr@Ž@ƒn˜PowerLawPSR J1036-83?ï]Ó¬~½d?–k§þ=0ƒ?"EŠw‹t?–k§þ=0ƒ?ë=ÂÀ{Ó?½õ¥;ÁÕ«?Ãôþ³ú?½õ¥;ÁÕ«?í_‰§Öj¨?¡ê`I+?µ²ÁºžB?¡ê`I+?è:P7>ÊZ?¡œwʅØn?Ï¿#֘?¡œwʅØn?íŠñìIa?¶ÀÕ<šÖ?³¨pŸjâú?¶ÀÕ<šÖ?ÕCÃ+ìËx?іèÏ·¸¾?å^j	šD?іèÏ·¸¾?èBJìýÂ?¸L†'£,Ë?ÎöÔLàù?¸L†'£,Ë?ÈúR‡óe#?¨Pè/H?éÁk^&·?¨Pè/HMIXED3FGL J1037.0-2934@pî¼ßï¿@@8Ïà0VàÀ9¢<PgÀ;‡vG…?ï­Ýò ,A@δMÏì'@½æ¿Þ}ºüüщ¿èGL'!L£¿äŒgv©!¿ïÿ =Z~AGNfsrq@‰K;˜Çâ'PowerLawPKS 1034-293?ïýIñxu?;þœ¸¬K•?5°róúû?;þœ¸¬K•?ïnö-­/?Õú•)¾?'!>|(%?Õú•)¾?ï^"`8‹?…èÒe2ÌÀ?"-ŸËaè¨?…èÒe2ÌÀ?íäú¨I­?†îmhØ?°Ø*»úÉ^?†îmhØ?ïý<9IÖ@?;­ÀfÄe?67"ý€<?;­ÀfÄe?ë'»òE=ˆ?ÀaW78?P?Ãa6ë	à?ÀaW78?P?ì%?™ôt§3ðy?¥u14ŸQ¼?™ôt§3ðy?åq•Úå%?°Ñæ¤$½?ÕÔàJ5·?°Ñæ¤$½AGN3FGL J1037.4-3742@q9Ê?‰'Ë@1òŽ AS‡À:*®í¾´ÜÀ;ÅÌðÞúÍ?ÕêêÞÊj@ä4i>÷@
îßòŒ¿èb^<¿æ/Y^ëô¿ë'lkZŽc¿ïÿ9M(¨AGNfsrq@{$÷ãÑÌPowerLawPKS 1034-374?ï›Oÿ>0Š?¯Ù!̆ëg?‰,3ãy?¯Ù!̆ëg?îqC¯º?ª¨vôV"/?¨ëÏ·ÜÒ^?ª¨vôV"/?î‰'ש?•Ë‰D¦'é?§o—ãB!f?•Ë‰D¦'é?ëØSÍÜ|?ž~ª‹çý?Àž°Ë Ž?ž~ª‹çý?ïcF"t?£í_Íò›ü?sŽŸ
ƒ?£í_Íò›ü?àmÀx^>?ӌ#}T•?ß$ÄC"?ӌ#}T•?í‰+që!C?£"ùsSF¿?³¶¤oËé?£"ùsSF¿?ʙ¨ó~½J?°2¡sä›?éY•Ã P­?°2¡sä›MIXED3FGL J1037.5-2821@päo€Uûµ@9☠uUíÀ93Ád¹½üÀ;€C_?ÒïñŒA9@Õ Û,a@ñºÃ.¾¿æ8÷׬=¥¿åáJ‡°Œ¿é®÷!F¿ä"\@?-AGNfsrq@‡a°‰ 'PowerLawPKS B1035-281?ïÿz7îG¶?!Fï—æ?¹
nŸ:é?!Fï—æ?ïÏÍÓ]	Æ?…×ç³Ci?xVJÐ?…×ç³Ci?ïÔIÉ!Ç{?xwPˆ?uÛw[Ru?xwPˆ?ïÞë!Ãìv?Rå¹O8ï­?pŠo	Å?Rå¹O8ï­?ïþí?wÓæ?"­·r˜ú?!,@É"c?"­·r˜ú?îó
ùz¢*?©ù¡b­ø‹? ÏPjé'\?©ù¡b­ø‹?ï£ýåb_?€=Äʲp?~®Ïp®?€=Äʲp?îo-ÌG?•ÞýÄ8?©
.4ó\?•ÞýÄ8AGN3FGL J1037.5+5711@bùŸ˜=@Iáü`8NüÀ8<ÃÕ­FÀ:èâï?õ.HËùp@¡½Gɘ:?ù!†â-\¿ÓS'¼Ä¿Ü,+³sE®¿Ù[žÔA
¿Þë·V¡öAGNbll@'¾ùÛ"ÑLogParabolaGB6 J1037+5711?ïþ‹'™f³?"ARV²Ðo?'GÒ¼f@Ì?"ARV²Ðo?ïÕ퍳K?}PøßÝó&?u	Ѓ²E?}PøßÝó&?ïK4Š~Ò?'%ÆÅ~?–žùk@‰Á?'%ÆÅ~?ïjÉÜÁ.?p_~š)¬`?'¦ßæ¨>?p_~š)¬`?ïü'<$•Ù?A¦d#"?;n}ëª?A¦d#"?îç]7FEè?®f¯Í½¬?¡Š,‰ì'?®f¯Í½¬?îÿˆN»?œ¾uìÍ;? {¨h‡?œ¾uìÍ;?îIä{b?˜^ø\=[?«oŽâ"0å?˜^ø\=[AGN3FGL J1038.9-5311@q¼ M@·o?ÓՀÀ8-¿¸èzÀ;)iϧr ?úÆbã$''@F5‰ÏÍ@#Qv?Lq¿ã¤˜";¿è@;ªóV¿ë'ÞFz}¿ïþè"IŒwAGNbcu@tuÔ`ªdÃLogParabolaMRC 1036-529?ïÙìqþ?qÎǺp?s	öúvìÚ?qÎǺp?ïá÷à?—Q?˜\û?Œ¸Ïøwâ?—Q?˜\û?îRy0\X	?œ&°ŸÃÊÞ?ªØlø'±k?œ&°ŸÃÊÞ?ïíÆqÛî?Må纉µ=?b9ó¸¿9¿?Må纉µ=?ïÂzMùÝý?|âûÒ¼­r?~ÂØ÷bU•?|âûÒ¼­r?í)Ï~¥Cé?Ã~àÁÝk½?¶±"®´?Ã~àÁÝk½?힥žîÕ?£ýǃN?³
Ó
Þ®Ú?£ýǃN?ïá,çOì
?gEc¼.ñ?nÓwº[?gEc¼.ñAGN3FGL J1040.4+0615@nXà†8@JE»üÊÀ8Ñ:6\³_À;x§P;¶?éq‰žò@OŒ¼çQˆ@ÏgÀƒ"H¿áø~«E'Z¿ãõ1Tƒ1p¿á÷,̑é¿èÑ2uÚAGNbcu@uv"Fs'PowerLawGB6 J1040+0617?ïþÍ­óBØ? š•ôã?#%žŽW? š•ôã?ïÓ—aÂ#?€G¹Ûäî?vs´c¼–]?€G¹Ûäî?ïáAÝß³s?t'¾¨ž!š?n¾"LGŒ ?t'¾¨ž!š?ï 	䘊?e›T¨Ô˜?‡ý»Í¹g?e›T¨Ô˜?ïþ&­OK?2¢yú—òÊ?-•,Ð:G?2¢yú—òÊ?ï
Í%7G? †&tXÎk?žF[\†¹y? †&tXÎk?ï­"l*dq?‰¼}9à£#?"·d²?‰¼}9à£#?íÔ»N Ž?›!"T"\^?±Z#"³?›!"T"\^AGN3FGL J1040.8+1342@lÄHS'^@L]⟜èÙÀ:¦–À¡E`À;×Û©¢f?Þ¸4r@–`Þg)?ü(ôÀÜ©?íó™Úç¿îö'LdÌ?ë@"!'÷¿¿Þ «ˆìAGNbcu@³·Ú=p£×PowerLaw1RXS J104057.7+134216?×
y'?ÊG…|Î!?§erŒÄ±ç?ÊG…|Î!?ïÜöQÅ3j?€,WzNöi?q"×?v½?€,WzNöi?ïəÀʤÃ?€iÓ¥Nn¦?{3Š/~~?€iÓ¥Nn¦?ïëÃ}vV?\Ñ;ýø4û?db<hl¢)?\Ñ;ýø4û?ïý:Ÿ§êY?Mìüó5ÉÏ?6+¢oA?Mìüó5ÉÏ?ï(	£º&N?¥»F`¹2¤?šþˍâ ,?¥»F`¹2¤?A¤²t?‰Ž"ï?ŠÕ¯ô+?‰Ž"ï?ïßfCÖ¢?{"›²´Vä?pLòÃG»?{"›²´VäAGN3FGL J1040.9-1205@p<>_·¼@C͆_¡PÀ:_Ü#åHÀ;×m‹ô•i?Ù)EÝô6@s¨(}¢˜@ÚßVø4¿ì	uéªíÄ¿¹e'»ež¿á`!œn¿åÞµ'ƒSAGNbcu@¡Œ"ýó¶FPowerLawNVSS J104108-120332?ïÿz¹|?Ó"瑖ƒ?0§¥n>u?Ó"瑖ƒ?ïѸ)Æ?ƒÎÌë—?w#ùí‰á6?ƒÎÌë—?ïä6'À[?q–ŽÚFZŸ?kÉ}Ê+›?q–ŽÚFZŸ?ïνë]†™?Wèsi°š?x¡
iI÷n?Wèsi°š?ïü]øÈm?A'deZ?=:}òï?A'deZ?îÙVäÏ^3?¯ÈHÒ®m?¢j'±RNÖ?¯ÈHÒ®m?ïÔÒx;¾?y]^]4	Ü?u–ÃòüÀê?y]^]4	Ü?îc'Wü·?"ÿ—$tS?©Çڎp4Š?"ÿ—$tSAGN3FGL J1041.8+3901@fšž`=Wy@NGU?ÍuiÀ:Ò2Ò»#WÀ<]€
×Y?âUÁݧÝÌ@
÷œ{?ÿ'dÿ^'?ïþæj­ž¿ÍÀ…¿z²V¿æÙ«<%¿Ü×k\fÖAGNbll@¤pžùÛ"ÑPowerLawB3 1038+392?ïø ô'ö?X+œÎF?OÝ{!lD‡?X+œÎF?ï"ÊÔ,Æ?Ž¶ú¹«C ?Šø
JôÎ|?Ž¶ú¹«C ?ï;(–]`??Žá8e5?˜ší-tÀ7?Žá8e5?î0g0»´¢?'ÿ«
¸¹ë?¬ùŒñ±ë?'ÿ«
¸¹ë?ïž]í	ó?Š¶¦$)q?ˆhsw_?Š¶¦$)q?ëu}c5·û?ÃúsßSk?Â*
s) ?ÃúsßSk?í郟1^?£—wa}¡Ö?°³ãã ?£—wa}¡Ö?áåΑ{›Š?ľéœt§?Ü4bÝÈë?ľéœt§AGN3FGL J1042.0-0557@oֆÀ
¡©@F:ØÀ  À:kÃ
0j+À;ÎÃÍIÊN?òi´Ï€t@
Í."®×?ÿr?7£Z¿êﴈ³Bb¿èJWqMl'¿¦ÛnŒ`Ý!¿ßˆùiÊWAGNbcu@±Ýo²-PowerLawPMN J1042-0558?ïác¥Ê]?w¼ÐQýÓÊ?nœZ*¤1Ž?w¼ÐQýÓÊ?îþ}Gd©´?¦•lSßQê? +%»?¦•lSßQê?îÐ~ùdõ?˜k{+'?¢øsÙLª?˜k{+'?în¾`9?'Žíz3¦4?©Dùül?'Žíz3¦4?ïá Ý"ãã?xÀúd°
?nß"þ\‹?xÀúd°
?æüpV²ÇÇ?ËR¾ÿ.ÉÂ?ÒRšps?ËR¾ÿ.ÉÂ?îN>sGK?¡;Pˆ	¢Œ?«ˏM?¡;Pˆ	¢Œ?ê5ì$ù+?¹þÿ¶_Å?Ç(OlS?¹þÿ¶_ÅAGN3FGL J1042.1-4126@qf1Ào@.cŠ '§À:˜PÀ;äcâ'§å¿û!tïÁ@b=OçÉ?ÿž/ÀâÞ²¿æÃڈ!L+¿èiòX]ËH?½ž‰`™üI¿åë®ïí
_AGNbcu@¯áУ×
=PowerLaw1RXS J104204.1-412936?ïÿ^F©©ÿ?ïm½?7)NÂRç?ïm½?ïÐ~Ó£x?ˆÄ€Ø?-?wÀô'¾§ÿ?ˆÄ€Ø?-?ïí…s¿6Ù?P«|ñœRÅ?bzŒd…Q?P«|ñœRÅ?ïÿö_Ã4>ʓ­Èß!Ý>Ó@5ϋþm>ʓ­Èß!Ý?ïÿ!넕H?÷]Á¤#Â?ŠÛu¡œ?÷]Á¤#Â?îê"Ó¹Ðò?µÅ¡YË[/?¡W²Ã‡	ç?µÅ¡YË[/?ïés»RjË?i¤Ûù±Î?fŒDÑQ%?i¤Ûù±Î?ïÿ˜n¡He?†5;¢Æ©?	ä_Õ6ñ?†5;¢Æ©AGN3FGL J1043.1+2407@jsˆ M@NÝÀ:SÀ9l5Qñd\À;²£á8k?å-ÇêB‡@"iÞ @ðO@Z
=¿ÙÿŸØwûº¿åSâì&Œå¿ä@½€­Ã¿åŠRĝÿ/AGNfsrq@'Sx}¿HPowerLawB2 1040+24A?ïü³	WA°?@c³É½™?:g·Za?@c³É½™?︭´'B?‡©IÖ[îs?Ôœ¿ç†?‡©IÖ[îs?ïÄØlñ£y?|"õÖñ?}"É‹ý·??|"õÖñ?î;½:*É?†ówi? ?¬D,_p?†ówi? ?ïï5´åð?cá\?ÐU?`ÊKć˜?cá\?ÐU?ëñXê>'?Àm¦p0ƒo?À:ŸèWº?Àm¦p0ƒo?îÄ¥h|7«?S$¨Œ?£µ©ylI?S$¨Œ?âYe+JS?¶:X¬Äœ?ÛM5©kYü?¶:X¬ÄœAGN3FGL J1044.4+8058@`I¥Ò@AXe_Ö)mÀ9Àû¦ÔëÀ;\íbnŠ!?î3€FêÜ@™¬Ÿ°´é@"ÀŸAú¿ØEÛpBw
¿ë$¶-ׇD¿ê:` |!d¿ïü9®;VAGNfsrq@ŠWÄg8~PowerLawS5 1039+81?ïâCV–åŠ?­N¦(¹«µ?m¼©¥"•y?­N¦(¹«µ?ïÃeÒ0¨®?…"¿$f?~MÙí9?…"¿$f?îΡM9'?"ö˜âµMq?£ë/֊Ð?"ö˜âµMq?ïAç'1,?z<<+ƃ?wÃ
¹ÚŠ?z<<+ƃ?ïýÙ<ÐH‹?11;Ñöœ?16Ÿra?11;Ñöœ?î9ð™É?°jðEW5?¬g ô·åo?°jðEW5?îw‡/~b?œñÅMÔ(Ÿ?¨‡¿›Îã?œñÅMÔ(Ÿ?ê¡`Ò§{?¬"y³?Åz|·¥b?¬"y³AGN3FGL J1044.5-5737@qé2`o¬`?òx W À6·èɂ•qÀ:BÙ­…ߨ@z—ì¯@aP!«vf@~÷€—:¿ÞÀõ0̯¿äT]ã
%ô¿ç
€û¬Íî¿î‰ÿJÉPSRPSR@÷6®}VmPLExpCutoffLAT PSR J1044-5737?G÷,íÆFV?RãGØÇ°?ïú4¸™d?RãGØÇ°? «´›Ÿû€?¼½*uýç?îõD¶FH?¼½*uýç?±öÝ êÍ?£]M¯ë~?íÜ!$N$6?£]M¯ë~?da*Ê©eû?Rž¨Ûٕ•?ïëžÕKT?Rž¨Ûٕ•?Arêp8	??Q¥ïsz?ïû£EP'q??Q¥ïsz?Áq‹ބ?®}>~'?ï€ú9Ӝ†?®}>~'?'O4ê¬?'Þ%¾H?ïm‡fmë?'Þ%¾H?9~Ibxª?5òLO½di?ïüÐ6Ój?5òLO½diPSR3FGL J1045.1-5941@qù±_ˆü"¿äB% 3ÍÉÀ6´ýÓÕՊÀ9­Õ~L69@z§3
C{@4ü(+?ýÇ3½G¿Ò`x:Ï3Ú¿äÆëvÛÿp¿äˆ§¾öJu¿ç.†%HŽåOTHERBIN@©££¢œwšLogParabolaEta Carinae?³G'~•ŸI?¿º¼BÕ¬^?í—°;
‡?¿º¼BÕ¬^?¤Ç°äQ`?¿ qU?ñä*Ú?¿ qU?Ò00ŸZ"á?³Pu¶«ò8?æçç°Rî?³Pu¶«ò8?°Z}Öü?''"—8r6?íìT°-É?''"—8r6?·ÿ-6è›?È‹BòK•?íY?í?È‹BòK•?‹ûRØPJ?ªç»gT
	?ï"è´ž¿?ªç»gT
	?Ü)ö꾶p?·Ón?á늠¤È?·Ón?‡¹µ"I¡?y•'P
¶"?ï¡+[^²?y•'P
¶"PSR3FGL J1045.7-2926@q	ÜÆø@9îσ³~À9:kÕ;0XÀ;"'»0?â"Åù/<•@œÈÿåí@¥bYât¿æ(Bn1y¿åÍa1É%οä+RÉGÿj¿ïÿÒ1ª`ÖAGNfsrq@‡w($xPowerLawPKS B1043-291?ïþüæ¬-+?©*ʛ§‹? 1'Ô**-?©*ʛ§‹?ïÙÅÖZâq?€ç»ìü×O?sÑ.ït?€ç»ìü×O?ïžýL­"Þ?{!.3|&À?ˆ@¬ÊL4¤?{!.3|&À?ïý'¢:?!eF3PyD?7+|™À¶¥?!eF3PyD?ïÿÁÐß?)n¯©yt?<&Óÿž?)n¯©yt?ïL¥Î8æ.?¤~ôùLî¬?–kF>
¤4?¤~ôùLî¬?ïUbº½ý?'`¶Ï	'ü?•S¨®r_?'`¶Ï	'ü?ïöõâ·ù?J_Ÿ8!æ?R<W,å?J_Ÿ8!æAGN3FGL J1046.9-2531@pèÙ'ÿ@=gqß@lØÀ:'8§ç:6À;ÉÙ³eº?ÌW'2_@cü3?ýŠ¿_&?궾ä½ëo¿â]'ÿ´'Ô¿Ä'ÿz㺿¿æJ£Ÿ#h²AGNbll@°vÈ´9PowerLawNVSS J104651-253547?ïþ)‰³•?-é
u2£?.iÊM»,?-é
u2£?ïÓáæ±Ç°?zh…¬¸ì?v <ï÷?zh…¬¸ì?ïÓÀþ¸ß?sëœk'"?v€üÒ<?sëœk'"?ï°ðÊû2Þ?j²A~Kº?ƒÃÍ>¢~?j²A~Kº?ïõ󯏥$?Xr(jó	?T¡VèG9?Xr(jó	?îʙ
O^?©{=wª''?£Vo'Ÿ?©{=wª''?ï©>‰—\Â?…$;ö‹?…°]˜kl?…$;ö‹?î?¾×õ''?6ßl?¬џÚ?6ßlAGN3FGL J1047.6+7240@`׆@ €@DÀ¾ß¤?æÀ9ž.§³7ÐÀ;²Ä§d]x¿ôêeI/ôº@òfsÒ_´@mŽo¿ã~¢zòB0¿á币Õò¿à—í+ð|¿à*'ßB	AGNbll@¤œçæšÔPowerLawGB6 J1047+7238?ïÿádçé¼>åkËÛ">î›°ÐÉ>åkËÛ"?ïçØåó?k·m…å•Å?h'ú@ˆ'K?k·m…å•Å?ïòpÚÕñ[?e g¸!ÏF?[JÏÏ9"?e g¸!ÏF?ïÿò0´}Ì>Ñ·±(=ä§>۞uza>Ñ·±(=ä§?ïÿØúúÔê>î¥)[ Õº>ó'š.²÷­>î¥)[ Õº?ïQ
=_uË?¬0RÚÍ©\?•Þ¸Zð~'?¬0RÚÍ©\?ïòXx£;?g¥S"'?[O¹‰×?g¥S"'?ïÿ8
§LN?õÔ¼¶Žs?þSxDÁ?õÔ¼¶ŽsAGN3FGL J1047.8-6216@r"ŸºEÀ9µ ÝDÀ8-r)HÀ: †ˆDÝ?öoôǽ™S@í/çú$Ê@<|z¿ãðÒ
¾¿èøò;‹
N¿èrz_'éå¿å3ø·P'¤AGNbcu@[~ùÛ"ÑLogParabolaPMN J1047-6217?ïû{vmðs?DWo'.ø-?B%k=¹Ù?DWo'.ø-?è²­'ÀËH?ƐH-§i?Í5IôüÒà?ƐH-§i?î½to
Y?œØ"L?¤(¹Íæg?œØ"L?ê8ä(ÈÙ?ž-ʘ³ù>?Ço_¼Ü?ž-ʘ³ù>?ï¹${?ŒQµS8?¶øÕâEÀ?ŒQµS8?ÇJYµ¨îÌ?ÃT&↷.?ê-i'•ÄM?ÃT&↷.?ìÑßÐN{R?©|!—?¹q~Õÿï?©|!—?؍IPù94?º^Ôéj¬?ã¹[Wƒcf?º^Ôéj¬MIXED3FGL J1048.2-5832@qöíÿ'+¿?⏣?Ïg¡À6Sà_PÈoÀ:ü¨\ªü@.¥5¯v@%¼`CÃ@¢ùš
WÈ¿Ô¸…Jµ¹¿á_6›L¿æs7ò#=¿ì8w{ó§"PSRPSR@<5%F
¦PLExpCutoffPSR J1048-5832?8üî\Ž?6daBšZ«?ïüà~'·?6daBšZ«?¤9ä>Â;?ÀÙ\æh‡Ü?î¼a»íè?ÀÙ\æh‡Ü?†U9D#®K?‹ÊÂ]<"?嶺Óôg?‹ÊÂ]<"?Umu‰"Ò?Côuôls?ïõIEnI4?Côuôls?3Žìq"q?'㴖÷?ïýŽ"d{L?'㴖÷?…Õ*[¡¥ý?§ñ–<º<õ?飼VŸ7Ø?§ñ–<º<õ?tm9aqS?`g'µ[V?ï×%!Ž?`g'µ[V?-l,;H?+'½Ú@Ëì?ïþ)>p[»?+'½Ú@ËìPSR3FGL J1048.4+7144@`íßý`é@E#,?ùëÀ8ªE¹GµÀ;jä'Ë÷»?ð"……æ^n@hðÎ3Õ@"m`*¸¿âp4؜0D¿å·oK
¿è'µ"9¿æ€¾;x.AGNFSRQ@…ʧ-PowerLawS5 1044+71?ïÿ#b@ù?o	yƒ«?"¹®«…E?o	yƒ«?ïÌ	ùÃ?"gt*a¹í?yþû	¬jA?"gt*a¹í?ï¬éœÞ"î?"}«Û,?"Řҩ˜†?"}«Û,?ï7õǏB ?{™u@ìO?™G«ÿ?{™u@ìO?ïþÐÍÒ?0²_7S~?/rïT³8P?0²_7S~?î¥{Õìä£?¯#ªüƒÎË?¥¨B¡1µÒ?¯#ªüƒÎË?ï]G…·?¡Ë0._Ô?"Nð00?¡Ë0._Ô?ëZÎæ­Ò?°rˆŽ¨{"?"ǀeH¸?°rˆŽ¨{"AGN3FGL J1048.6+2338@j¦ôÿ†]}@O/ »èÀ9¹i,êCÖÀ;½WQ­D?ív½µhé4@?mÚÎî@Nvÿ»·|¿¥Ÿj7_¿çÏà0½ô(¿â͉:¦Äû¿íY¡ÃAGNbll@'N͞ƒä&PowerLawNVSS J104900+233821?îîGg·c?¢'щã?¡‰ö4?¢'щã?íLdå‡Ù©?°¼C͆Ç?µœØÕ
9?°¼C͆Ç?ì¢G4ÇÞ?¥t˜æÜ)?ºï]ÆYÁ?¥t˜æÜ)?鑧V_vø?œ¿XM§†J?ɹb¦'$!?œ¿XM§†J?í®™x	?±ê;ÏbI
?²8Ü
´?±ê;ÏbI
?â¿LmZ»&?ÍÅH‹¬hv?ځg%J‰³?ÍÅH‹¬hv?烽KœØá?¸øêþµ
?Ðø…hÆN??¸øêþµ
?ÑÝê6?,;?ª/44µËF?ç
äàiã?ª/44µËFMIXED3FGL J1049.8+1425@lÝ¿˜0ä@MË@ÒÎÀ9÷¿µ'À;˺µsô?Õ>vn3@Ëãæ™Òz@¨‰?"O[¿èÈ蘟¿ã€ßxöáÉ¿ã<æü+'³¿ïÿÏ7؀×AGNbcu@'c‰ã½PowerLawMG1 J104945+1429?ïþ»l}+Ð?5Fvšv?$I:×ÎX?5Fvšv?ïÚÛ~ýrB?;㲡»B?r'@ŠåÆÌ?;㲡»B?ï_8MŠˆ–?‡p#WÇÑ?"öUŽ%=?‡p#WÇÑ?ïÁæ0îVØ?a¿4hÔ^?瘢È?a¿4hÔ^?ïþèÙây?7^àF?Fõ?.ÁqXšû?7^àF?Fõ?ïˆê[U?ªM;tU?Ÿ®â»}m_?ªM;tU?î6 †Ùߖ?¡;
µ.Ò?¬•÷'† ?¡;
µ.Ò?íºp.ÄÂ? nð|È?²,~‡´-³? nð|ÈAGN3FGL J1051.4+3941@fMp€0<@OjÀh:|À:s0V	!À;¸Ir9Ù@?Þxš¼ü˜@
—ÉøÜö?ú¡I …[Ÿ¿ïÿëü¨:?ïýøÞp¿ܮ'@òʟ¿x¶0d]ÿAGNbll@³(âe,PowerLawRBS 0909?ïþÌZgP?ó#£Ô†?#:_k5?ó#£Ô†?ïÞ96,ŒÑ?…
n¹'Ê?pãe
µ×c?…
n¹'Ê?ïߚ¹n?eRÿÐ\?p2£^õôÛ?eRÿÐ\?ïâ¤æ\s|?YkðIļ'?m[²ªËê?YkðIļ'?ïûº2bË?A.­|Õà?A6¶?KÎ?A.­|Õà?ï¸?ïP¨?°"'°ã§?(ø^?°"'°ã§?ïŧ:Û·æ?|j&×0±)?},b–ó€ü?|j&×0±)?ï$­D#ùã?"‡Ô*?›jWt¡‹­?"‡Ô*AGN3FGL J1051.5-6517@r-'Ÿì™òÀÐ3³À8ҙ!¤•vÀ:ñÅÒ݈¿¨~".xðI@û)/y?@Äb¦-¿åÜ©ì£ö¿ëú¬{ôm%¿âúðcLM¿àš_ð´AGNbcu@‰?ª šª;PowerLawPKS 1049-650?ïó×C%ø?`ñŒá?XQy\ÖË?`ñŒá?ï'D¾uñõ?žâìÇÓX?‹®ÐibºÍ?žâìÇÓX?ï^ëÝ«Ž±?ŽŽ¤íë?"""LE÷Þ?ŽŽ¤íë?ïéÒxw#è?M§G»$?f-‡m_8|?M§G»$?ï´1ª
ï·?†KèøÌ?'󕁻<?†KèøÌ?ìBऽ[?"ÀÏ=•b?½èúÚ#—?"ÀÏ=•b?íã9K¿?¡¾à8Úÿû?°æ7ØK•‡?¡¾à8Úÿû?îõXÀ3—?Ž
Dy;1-? ªt""?Ž
Dy;1-AGN3FGL J1051.8+0105@oD  ô×®@I¢¹¿©Î›À:(48ñÀ;¾º•"<¿ôÉ&úë™@¾g'‰«@…n€;N¶?à<LCûWz¿èuzýŽP¿Ñ蛡¿ãÙÝu«A§AGNbll@¤õ$ÝPowerLawNVSS J105151+010312?ïþ2ÝË?EÛ"êù?(á%<õu?EÛ"êù?ïÜËùNq?"õ¹L‰½Ñ?qÀ÷ªt?"õ¹L‰½Ñ?ïÑ4Ú
ŽD?wÑ?Lïæ?we"ÆÁË?wÑ?Lïæ?ïÿ-¼?¥¡?րµV?H{'W½?րµV?ïýÄæÆÀf?=ÞâÙû!?1ØÈT'Tš?=ÞâÙû!?ï9X¢"¦?¨}ŸƒŒ"¬?˜Üôï6?¨}ŸƒŒ"¬?ïÃАä¿?Jjg ?~ð²¾,n?Jjg ?ïñMÏãúÞ?_ºyn$?]d`'¿ó9?_ºyn$AGN3FGL J1052.8-3741@qf[@-¹@3uÑÀQ"GÀ:Aµˆ©\À;¼óË>WT¿ûrßsB—Õ@ˆnÙ§{¯?ÿðŠß—¹¿êք4ò>æ¿áž0I@]5¿Ò0¡Ðl6¿Õ-îƒ^wAGNbcu@§óp¾
í)PowerLawPMN J1053-3743?ïþØLª?—Yì.W?"{5…£u$?—Yì.W?ïÔ'Öx?…Ú‹¥ÒÞ?uõ7{tœ?…Ú‹¥ÒÞ?ïãeG,?i•­;6?léšx:É?i•­;6?ïÿò6œQã>֊;n>ے'à"Ñ>֊;n?ïýîb@P?+{Cʲy»?0Œð%ÌA¢?+{Cʲy»?ï*3Í.hë?¯iÖÍö{D?š¹†]¢~?¯iÖÍö{D?ïÜÓIyØ?s# ¤ŽâÖ?qû–S*?s# ¤ŽâÖ?ïþã{BŸ?"Ÿ­Mì?!ÈMN(t?"Ÿ­MìAGN3FGL J1053.7+4929@d*à~Zy@MŸä6vÀ9­µ|N/8À;'
ãˆÐôÀ .s±@mwô-cæ?ü»È€aå"¿èˆÂ¬bt¿Ð¹9#¯¿Õ,¯Æ¯¿á}"ð+2AGNbll@¨Ø—Á½¥PowerLawGB6 J1053+4930?ïÿ*Q¯—?r¨åõǛ?µÆÉo˜?r¨åõǛ?ïê¬Q¤…?p+":ߖÕ?eìSðSúÓ?p+":ߖÕ?ïç_Í<€±?mY(ßI•?h 2†Ï$?mY(ßI•?ïÿýÄÄô>µZíàõ>>±Ú™‹
F>µZíàõ>?ïþ|¯upg?%ªÐžßç?(5
}]è"?%ªÐžßç?ᓥ±?–+Ά»'?‹ßG¥eg©?–+Ά»'?ïà¿†?ué,]7ßÜ?obù_(	Ù?ué,]7ßÜ?ïÿԚ‡¼^>ýwî!ÓÞ¾>õ²­Áˆ"¹>ýwî!ÓÞ¾AGN3FGL J1054.5+2210@k!«`kz¢@O‡@`B_÷À8ÕE!r@À;'°Ql^¿òž"•P‰°@¸'uåµQ@šþ¢Lœ¿äÒÒË?¿ä M¼¿âJˆÝ½=–¿à]Åsù2BAGNbll@'ÒDЩPowerLaw87GB 105148.6+222705?ïÿÔ/‰>êÉ?}ü>õú]u	C—>êÉ?}ü?ïäqçxõŠ?Â³CK?kŽ_.þ?Â³CK?ïîrŒ9‰¹?i
â«V;"?asÉ5ö?i
â«V;"?ïÿÁú"cØ>õFCŸQÀm>ÿ««:è÷>õFCŸQÀm?ïÿՇJPu>ñ¿-vˆÐf>õ<Y_Ly«>ñ¿-vˆÐf?ïiŸjWÑg?¢b'ÈR?'̽œÙ?¢b'ÈR?ïëS£É¦Û?r'£˜ž6?d¬\>˜4Ë?r'£˜ž6?ïû"ïÌè7?Aetk(²µ?A¬A˜TÀ–?Aetk(²µAGN3FGL J1055.8-6025@r*@ºˆ¿æ°ÿðCRÀ8>öJt˜XÀ:0ÞÿÕ7Õ?ÿ¸VÉ}÷@μlØE|?ø¥ˆX‹¿êYÆO°‰¿Ç;šNº"¿å8BhҞÀ¿íú±°=PSRPSR@£B\(öPLExpCutoffPSR J1055-6028? ÆÿËûUi?%½×CT•?ïþóü"B?%½×CT•?©É&F?À–Rt8ƒw?în.ӖÚ;?À–Rt8ƒw?»Úkœln?§%›A¥Â?섬RŒrr?§%›A¥Â?À.Qj¾¡? ï÷ãÊ?ëôk¾%PX? ï÷ãÊ?/$ô±6Q?&ºÒy;âU?ïþ
°}òÛ?&ºÒy;âU?‹<1xaÕ?©GHÓ~MÖ?~Ö¨?©GHÓ~MÖ?¦½#eρw?£–rºª?î"-ÉçÀ?£–rºª?"ºï(%¸?ƒúŒEĕ|?ïZ(†ö˜'?ƒúŒEĕ|PSR3FGL J1057.3-2341@pý8€®@@…ߨq¤À9ܕyyh¢À;·ûêlj—?ôgë†Ì7|@Âó5AU`@ˆàdõ"¿Í¹fb#zr¿ÙŸ
¦¿í~×?'ÄP¿Þ;Ê®d'AGNfsrq@Eœ¾ß¤PowerLawPKS B1054-234?îƒÀÊ
$Ç?³áŠìO‰?§ÃóañhŒ?³áŠìO‰?îÁ˜³?®tòm¶µá?¦óæx6ËÙ?®tòm¶µá?íe§ S®9?£dúÝB?´ÒÂü³¹?£dúÝB?ì¡ëԓ¯d?œˆOÖh=<?ºð¡[b"ã?œˆOÖh=<?ç•™|4Ñ?ͽbK¤™?ÑÂÔÍ–^?ͽbK¤™?ãÀ`¬¬à?Î䗎ý^e?Ø>¦¦>æ?Î䗎ý^e?é<ݹ¦w?±ÇŒûüe?Ë ‰f%?±ÇŒûüe?Ýr6¿ÀÛä?§nVÓT?áFä '?§nVÓTMIXED3FGL J1057.6-2754@q$±Ào@<{Ÿ³À:w•¤A"HÀ;ÌPwؕ¿ãÍç˜ÄÌ@{f°6?þ,TßÖ>æ?èvK6gΤ¿ã%ZºÇοß@‡ë­sҿ̎)‡ý~µAGNbll@°'©"PowerLawRX J1057.8-2753?ïþã)v'?½Iˆõ[†?!ÍmÂڊ?½Iˆõ[†?ïÚ²7†o?€ÖV÷#0³?r¦äào?€ÖV÷#0³?ïâòDì¢?aND*',¼?m
~÷Œ}ú?aND*',¼?ïÿ0îú
? Ÿ,îs?â"«ÓãÄ? Ÿ,îs?ïþ]ì-?1ò½èÿk"?/º,–-‡i?1ò½èÿk"?ï9ÜŽ.N?«ßvIâ6?˜Ä}1©Ò>?«ßvIâ6?ïÊ>îZï˜?~Ÿ"ÈìhU?zàˆÚWÇ?~Ÿ"ÈìhU?ïöϻзN?O
—©
°?R`ˆwN"P?O
—©
°AGN3FGL J1057.9-5227@qßÔ§e4@"àà*!½À5öU/}ÉÀ:—«bï¹a@JÝð
¿w@nFM—7•?ü,y¦Žu¿¸Ú§MXŶ¿ÜáåÂUê1¿éL)õØðÙ¿ï¥Ó–7óPSRPSR@…àÞ҉PLExpCutoffPSR J1057-5226?-‡P_Q?I¤Ô‰x?ïÿŸtI?I¤Ô‰x?£"AËTç3?ÁRÒµÄóe?îÇ»ã<ó?ÁRÒµÄóe?"ã|úm?'4B&ì?ïgˆä%ë?'4B&ì>½e<Ô>¶Ø/Ð24Ÿ?ïÿüSfô>¶Ø/Ð24Ÿ?/2ßPéÌr?%ã*Cs?ïþÒ:8Ð?%ã*Cs?ˆŽn2Ü£?¦Psú'q¡?ÆpoÝ?¦Psú'q¡?'^øÐ0?'0u¤)
?ï·²ƒöD??'0u¤)
>Œî::,I>'ˆƒ"Xb˜?ïÿÿŒ	/¡>'ˆƒ"Xb˜PSR3FGL J1058.1+7010@`ûrà\̊@EÿüŸù/+À9vëg†ùÀ;à±û.·¿ã§|p¾Ùð@Cٗá]¨@ŸÜ TsË¿æçˆûÅ;g¿éO>	X¢¿êùNñˆKœ¿äÆMy'AGNfsrq@}'Õ{Ç÷{PowerLawS5 1053+70?ïþֈo?)7F¼íÉÏ?"—zÆÝ ?)7F¼íÉÏ?ïß`ܟäÈ?€'çg(?pO'¦n³Ï?€'çg(?ïÖJÞ[ў?tEø¼M¦b?tڐê$tÊ?tEø¼M¦b?ïý6¢‡£?%Ý[õ@?6JìÍyöé?%Ý[õ@?ïýæêғ®?5ŸZdµ#?0È«{&…?5ŸZdµ#?ï9gì3«?ªÝܺa­r?˜Ó€iÆ
?ªÝܺa­r?ï°uI
éq?" Sq?ƒâ­Ä|ÑÍ?" Sq?ïÃ{&ß4?v&IÌ›?~~ÂQÃqý?v&IÌ›AGN3FGL J1058.4+8112@_ÿ+@öjU@AdË@ÒÎÀ9…Aî·Ù À;u¾¹å?Ù!Ââ,[@NiÔÚã;@T3‰M¿éò«ð"7¿æW˝;©h¿ëx`!ÿêYþQæ7éAGNfsrq@Š*cS÷ÎÙPowerLawS5 1053+81?ïþŸ|Ôß7?(9º0¸?&4;é?(9º0¸?ïّ´Ña?ƒBIÃ.W?s7%}2pÄ?ƒBIÃ.W?ïŸö•sR?"‡²†/?ˆZ´g·[?"‡²†/?ï÷m?5™k#[«²?QÕ%‹}À¬?5™k#[«²?ïþÄùï?&òç(]"©?#¾â»f?&òç(]"©?ïÅ_?®qªë,?^SWê?®qªë,?ï™@ß÷ª?‡ò¬Jð?ù?‰¾ï½³Ap?‡ò¬Jð?ù?ïÁîX+ª?pªË–y´?÷×YÇ?pªË–y´AGN3FGL J1058.5+0133@opŒ€A@Jc*`%څÀ7s\#íEÀ:µ#I±#ú?òè³ÍøE÷@Ð>â¾ÑŒ@碥0üw¿àã ïá¿äoÒBW"¿ã•ýmt¿ââ0-¼ž#AGNBLL@ˆ›V"LogParabola4C +01.28?ïöWº.Ã?hœ}
l±?SãP9+ÚI?hœ}
l±?ïØܲÀT?"XóŒq?sô'Àò?"XóŒq?ïŽrGZ?Ž"x˜ºn?Œcn-géµ?Ž"x˜ºn?ïúX=óo?1¤S³þ?GòžÖ·â¦?1¤S³þ?ïþ!ÃõÝ?;¯ÿ>M ?-ã¿ø­Y?;¯ÿ>M ?ïC3>?§m˜[lg{?—œÿÑfM?§m˜[lg{?ïfCü?"øWºÝÿ(?">þÄê}?"øWºÝÿ(?ïóI7EUc?Rô÷Å;6w?Ym'-ÝYr?Rô÷Å;6wAGN3FGL J1058.5-8003@rŸìºËCÀ2G?}ÄQÀ8%ðT'RÀ;*sMÕué?öfnSŤå@Õ	2®¨õ@óaDéi¿ÝÛ³'×hæ¿å¦,áÉ¿ä‰][û©Y¿çØH»/ÛAGNbll@€]Þ~¥øMLogParabolaPKS 1057-79?ïú,áÝ?Miã÷x?GLz}Gå?Miã÷x?ïšÿvS•?›ê'¹Z?‰@"k ¹?›ê'¹Z?Êæ?…»Óý®ò?ˆ˜þ¸.™?…»Óý®ò?ï¸äcâå?c•yŽN?Æýè¿Õ?c•yŽN?ïônFÛ?VÃôãI—u?WáÙh*z—?VÃôãI—u?íÂ<¶>?¾kŸÎä?±îJ:(?¾kŸÎä?ïî
uoª?—†­1:°a?œ>JrÒÌ?—†­1:°a?ï;ñqÇÃ?†Á\5â"?˜ŸÁÑÇ'?†Á\5â"AGN3FGL J1058.6+5627@b³fàé´@K8€iFëÀ7é´[¼¿9À;2¥n¹òÀ  :G¤"@'6MïÍ?ÿ€y¿ß)²_§õ¿à½0o‰z¾¿à;QÈÕ¿¿×'m½@AGNBLL@"n…‡"ÞPowerLawTXS 1055+567?ïÿý¬>ö;
Gc>þ!x…ªö8>ö;
Gc?ïè0^¨¾?{F»Ò†Ñ'?gÏ¡vÞ\Û?{F»Ò†Ñ'?ï×`ÆX-W?ã¢	~P·?tOœÍºS?ã¢	~P·?ïÿÿ»Ñ@¿>…,¥ÎD>hN>…,¥ÎD?ïÿ¨ã7??€N¡œ?ø,µv*?€N¡œ?ï€îó[Í?•ïhÞ.׫?ÄC*;Ì?•ïhÞ.׫?ïçœ SÿÔ?z´ÏæÙP?hcߧà¤.?z´ÏæÙP?ïÿûœÝµ—>Ìv±wP{>Á"E¤t>Ìv±wP{AGN3FGL J1059.2-1133@pšÑVŸ@EYá @è(À8AëÒK'À;4]"<?Þr!+û1@ÓrDëíN@qÀa¯r¿Þ¶šm¡e¿ã/ØñÚ^—¿Þ"]
]qÜ¿æîBøFAGNbll@|©á°‰ PowerLawPKS B1056-113?ïÿ¡âN¥f?VK KӚ?‡{«w¤¸?VK KӚ?ïÚj笈?'7:¤J³g?rÊý"óÔ?'7:¤J³g?ïë™<bÂÿ?bý…Ÿf¸?dfÃÛø«?bý…Ÿf¸?ïèPmD•Ë?L}ž]?g¯'ê$äÍ?L}ž]?ïÿÂ×Ú?]¸lPr?ç¡3#6?]¸lPr?ï]Uèâ$?ªÛ"•òÈ?œ´U?t'?ªÛ"•òÈ?ïè–þoî6?pü¬…š4?giÐ:4?pü¬…š4?ïU	ò?€õô{Îë©?ª½|y'‹?€õô{Îë©AGN3FGL J1059.9+2056@k'_ôö@Oî2à'¤À:kUž˜À;µÕЁ3?ê—×p¥ëž@gßbP­@Œh€Z¿éÌ,QÓÃr¿åÈãï(Ah¿î±}cX?é€4
AGNfsrq@Ž}ó¶E¢PowerLawMG2 J105938+2057?ïûu•"|?WNÈ»Ÿ@¶?B)©ŒAÉ?WNÈ»Ÿ@¶?ïÛgé@?"œ‹Ã@|µ?r~ÌjMú?"œ‹Ã@|µ?ïlgþ}/<?Š~Ì1óøH?'s5'|?Š~Ì1óøH?ïü9ï1s?<CíKÀ{?>0ˆA£¢?<CíKÀ{?ïùG¤s+?S¡"¾Ðê?K®áßs?]?S¡"¾Ðê?ï!²U¹V4?§‡˜Ü¢†<?›Éµ@>3—?§‡˜Ü¢†<?îHhFìÑ?ž
÷§{`r?«y{¡Iô?ž
÷§{`r?ï¤ìF?'dÏ\7þ?†Äøà)ŠŽ?'dÏ\7þAGN3FGL J1100.5+4020@eù«ÀãŠ~@OÌÚ`3F~À:
µÙk@ÁÀ;¹u.€F¿ê_hè™(@µù÷}?ý]À?u¶»?ïI¡¦¥¾
¿çÐ2ÈTB"¿áZœr€À?ÇàE²^.AGNbll@²2ŒàuöýPowerLawRX J1100.3+4019?ïÿ¨öý?…8Aî?øRIÂË?…8Aî?ïÙϚ¦ã?‹iX
I'?s2ïž
{?‹iX
I'?ïèh»ïõ?dæv½?gé—QÎ{d?dæv½?ïÿç¶z×>â%ZAç>èI¤ÊQ	ì>â%ZAç?ïÿ¾…GŽE>þ¡'7?^¡²gkü>þ¡'7?ïc›á?¨T"-5?"Œƒßݛˆ?¨T"-5?ïןM°‹?uכî?t0Y/^'?uכî?ïþ¨i7žt?)ÙÖUÃ?%ymL:Ù?)ÙÖUÃAGN3FGL J1101.5+4106@eÁŠŸb0@O½ÿôA†À:U€[À;Ð>åE¿ø¾"y@JDâˆõ?üK_¯+¿ésã@pw¿ÀƬ†J N¿Ûï kfg¿»|,êLmAGNbll@µæå$ÝPowerLawRX J1101.3+4108?ïÿ}–%=I?ùÐaÈ?M9‰ª>Æ?ùÐaÈ?ïåY¹.à=?€z´A?j¦FçBŸ?€z´A?ïêqöi?bËÇO›Ê?eûŽ6P'l?bËÇO›Ê?ïÿùE.eø>Å`9´R'>Êê¯[–!>Å`9´R'?ïÿEâk‰?t®Wš@þ?^æcJÂP?t®Wš@þ?ïmûœ »?¢&"/¸?'@Œu	e†?¢&"/¸?ïã—I]A$?mÄv\h¹º?lh¶Ûsû?mÄv\h¹º?ïÿ}2Ós?>™7!q?YŸ'Ôê?>™7!qAGN3FGL J1101.9-6053@r ¿p¿é±}À9rÀ7Õ8[' NÀ9Ò%çñ?ý'¤ö!d@	1‡úŠË @	¢®@D¿?â̤žZs"¿àW6³t ¿è…ÂÖ[¿íUç}¨!rOTHERspp@™tÝ}¿H€LogParabola?Q$;b†Y?ŸþQâÈM?ï÷mâSE?ŸþQâÈM?¢§°É!F?¿™÷H²‡?îՄó´?¿™÷H²‡?š¬'KŸï'?•§ÂJ@U?ï*›u£‡?•§ÂJ@U?ŽB"Úãub?ræ›|²C?ï†÷t¯ï
?ræ›|²C?&u—!3•? ßOEì/à?ïþžÇ­\? ßOEì/à?‰%]8"?ªôƒ®¢tœ?ï›jŠôvp?ªôƒ®¢tœ?}ký­~ù'?~8h›Üª9?ïÅ(Î=]?~8h›Üª9?Tµ¡<D6¸?FF+~¾zR?ïõ¥/h½?FF+~¾zRPSR3FGL J1103.1+1155@mÐ~KZ@N4_²?À9œ''%àÀ;Àæ"ß(¿÷ÒL%r€P@Eõa™š@#²`dä	vW0y¬¿çàVqH9!¿éFûzgص¿Üê¦+ù-(AGNfsrq@"}ç ù	lPowerLawTXS 1100+122?ïÿÅ/tŒÅ?¼œm>ýh)?ië"?¼œm?ïã†çݖÁ?ñf·Õ{ë?ly\"®Á?ñf·Õ{ë?ïä³Þ¿=˜?WËu¯è?kL!\?GÉ?WËu¯è?ïÿþþÖ½Å>—¤1*›"> ð%­5 >—¤1*›"?ïÿ³gS©Ô?	<JaIÙ
?&*¼³Ü¤?	<JaIÙ
?ïhùçô+È?¤¹•›ä÷?'àÂüS?¤¹•›ä÷?ïÏp˜:ì2?yu¤Û`Ë1?xG³ÉÌ·[?yu¤Û`Ë1?ïÿðªïÏ©>â–6Ýæ>Þªp{ŠÖ >â–6ÝæAGN3FGL J1103.5-2329@q×®6	@@‰¿¿ž!À9á¢çrÀ;lelkc%¿ì¼A/±Y»@Èvç'÷?úPúa¤¶?ïõz?ƒš÷¿ãx39W(u¿Ø;âŒÛ"Ù¿¶y‰âJAGNbll@¹"a@OPowerLaw1ES 1101-232?ïý5yØ?8
é"k'?6T7(p7Ê?8
é"k'?ïÝuÉÛ«¸?~§Ö™º[È?qE)‡{õ?~§Ö™º[È?ïÎï>'¶ ?s—K5[u'?xˆ`ÀÃ×Á?s—K5[u'?ïÿ H#I>ý[+­·¶y?íþiL7>ý[+­·¶y?ïû×4beÙ?CfÄzO?@£.ZëºÍ?CfÄzO?ï0ÙL?®Y[g"ã?™ÿ¤ÚM:‡?®Y[g"ã?ï©j·P[/?…¶½Ý>â?…¥R!š`g?…¶½Ý>â?ïûuU±Q5?C,UNË?B*©×iZÐ?C,UNËAGN3FGL J1103.9-5357@qöÌÈó#@—Þ_ò.À7ø_ð*ŸçÀ:׀·J"‰?óˆg¢Ñ{³@Ö[uòu@$6ým(¢¿àOéÜÊh;¿âý#6pY¿ã£¨™ÅA¿äfÈ\¶ËjAGNbll@ŠA"h	ԕLogParabolaPKS 1101-536?ïþ£6Pt?#þӋc¢®?%̙áxŸ?#þӋc¢®?ïÊ.ѓu? RV–¾±?º%͑e? RV–¾±?ï¶H]UµX?àÛ]Åi<?'mè®Eû?àÛ]Åi<?ûŒ?g7,4°?ˆP=ˋ°Ø?g7,4°?ïýbÑRåÍ?5ß`àõM?4étgˆou?5ß`àõM?ì¿;¹-wv?Â3_Ðá?º"6"DN?Â3_Ðá?ïMä¿¡…?"¤rª[Lœ?–_dœ3h?"¤rª[Lœ?î¦ÅLáì*?'Vؗoï?¥"«.q¡f?'VؗoïAGN3FGL J1104.3+0730@nµ‹¿PãG@Lõµ ÝDÀ9'UM9oÀ;­`˜ÇÃ?¡¹‡YQà/@ÖR²o@‹s'ÿÝñ»+5q¿æe ó$¿ã'åcË,¿Ù(•M¸"NAGNbll@"âÆö"FtPowerLawMG1 J110424+0730?ïÿ`ë¨/4?¥_>?â‡,ÏåÚ?¥_>?ïÛ)Èëµ?ƒ§ÊR'ÎÔ?rkt€%™?ƒ§ÊR'ÎÔ?ïï54•3?dÁ——
[´?`ÊË&ÍÔ?dÁ——
[´?ïõjP&ç?>B ™¸n?U+Õ+x!L?>B ™¸n?ïÿ8ÀÔ?·Å!{È?˜âÏGJ$?·Å!{È?ï!ü¥56Ì?¬îÚ57'´?›Àk\ÈÂw?¬îÚ57'´?ïÐããá?|•øtxQe?wŽwoSÇ?|•øtxQe?ïz±®Û—?"ǝïÜÊ°?©Ê­Öa?"ǝïÜÊ°AGN3FGL J1104.4+3812@fzv@c^@PB7¿õMõÀ5®à×E̓À9²‹-Æè¿àµƒíñF@æbu+?üX¥€'œR¿×Dû]õ¿Ýn(#¤¿×ÌæäŒBT¿ÔZ½#AGNBLL@'Œ'ÞÑ·PowerLawMkn 421?íÉÒ,:Ï?Á¹KgÔÇå?±±nM u?Á¹KgÔÇå?ïä琝q•?F¾ÒÏuh?koWª¡?F¾ÒÏuh?êäAÔ>cÇ?²-ýöš¹p?Änø¯pæ?²-ýöš¹p?ïÿþ³­I­> YÆôÕ6>¤Á(`öRy> YÆôÕ6?ïÁP)¹û?ˆN¬n/?WëDvBx?ˆN¬n/?ïx#šD?¢ao?T³ô?ûž0'??¢ao?T³ô?î£ßšÒ @?¡Gï?¥ÂT•Éú?¡Gï?ïÿýCb*m>»ÆZîÿòQ>µãmÇz †>»ÆZîÿòQAGN3FGL J1105.2-6113@r(ßÒc¿îðÉ'ÀÀ7å8ÇǪÀ:)óð?âö''ž!á@7Ý¢@v;Ÿ"X¸¿äƒAy$·£¿èbz–ý˜¿ííÃ3é3¿ÖÜßb]áPSRPSR@•´ä%®æ2PowerLawPSR J1105-6107?èê—^_?ÌUŸLi™?ÏÐW™¢††?ÌUŸLi™?ï$y'EÅæ?²5¿þ:á†?›pͼn­H?²5¿þ:á†?âÁÿ…Bî?¼û.p<_?Ú|õ{ö#?¼û.p<_?ïœl•³
½?r³OІ@?ˆäڝ‹dÏ?r³OІ@?×¼€ß?Òõ/+?ät!ú?}?Òõ/+?éuHƒb'?È)w¹†/@?Ê*Ýóªuú?È)w¹†/@?ßôrö1?ÄèË>h'?àƄøçw?ÄèË>h'?ëýk# ª@?²Pë:Å$—?À
Sq}Vÿ?²Pë:Å$—MIXED3FGL J1105.9+2814@i¢ß"xî@P«à"'À9¾‡«ÚÀ;Á¹žòžî¿Úãå¹þ@¹F–<lî@¼¾@Bo¿ç7âR1Œ¿ã_¾«e¸°¿ç½®J;ô‰¿é—ùUŽIQAGNfsrq@ØoÒòåPowerLawMG2 J110606+2812?ïþ/š;?14DËSà?-ã> ¿>?14DËSà?ïä‰ê‰–?'øoeÅ­?kvǙ²p?'øoeÅ­?ïµ±ñ1ä‡?€TýN‡?'"ƒ»Åî(?€TýN‡?ïÿ¸Cäí?
°ÂFr?èúÇN²?
°ÂFr?ïý¡Š˜Ž›?<'³¤Â?2ó«íªO?<'³¤Â?ïq|܎P?¢¨;Ú;?'Ü0[×0?¢¨;Ú;?ïRÇYŠ#Ê?'écGEê?•§ËKêÐ?'écGEê?ïõ­1.©¿?P¢CRåQ?T¥1ùR4?P¢CRåQAGN3FGL J1106.4-3643@qˆvŸÏ=À@5‡Fÿ˜ÑóÀ9e‹rXÀ;¡6Ç<j¿òñî»ÚŒ@‹U@¤4þ@V)«0ñ¿äÈé˜+ý¬¿äþÍGñÜ&¿×ä&íÌîþ¿ì1 x½ÎOAGNbcu@šOß;PowerLawPMN J1106-3647?ïÓýþÑ?wÏƆG'i?vD»$?wÏƆG'i?ïÖÊó6v'?"R¨í•1e?tš†CÈw?"R¨í•1e?ïH»ú'ßÿ?`ùðÌ?–耹L2 ?`ùðÌ?ïÿsžïU?0zFE³\?š}$7?0zFE³\?ïW³=¸$þ?˜ówDôÀ?•	˜B(V?˜ówDôÀ?ï@•9»û?£ö·ð±SV?—íXáؘ?£ö·ð±SV?írҟ8ƒÄ?§AR"ë?´ik…¼_?§AR"ë?ïòh%c<?U"}7›?[/ñÀ8H(?U"}7›AGN3FGL J1107.4-4447@qÃN?þó'@,‰9¡}ãÀ8ÉÔCédÀ;bŠ÷??åÕè K‹@…B(o@¶@ @&¿åݚ?½¿êõ†ÿ'å¿âK>}ý¿ïÿÛ*f8¢AGNfsrq@y•ÀëíúDPowerLawPKS 1104-445?ïþgÌ9vf?(û¿¸º+æ?)ƒ9:ö)t?(û¿¸º+æ?ï¾j¦^pp?ˆ†dLt''?€eV_tè?ˆ†dLt''?ï]S<)?‡£ -Íè?"Uµ?äÞ?‡£ -Íè?ï»B'¨'?c…¾†å¹?/[—ë@™?c…¾†å¹?ïþfüþÅ?0cGáœHw?)23½Ö?0cGáœHw?îfjÒ©'#?·dR˜†Ó?©™RØÝ)Ñ?·dR˜†Ó?ïècùq?•Ã£XüZ?ŸBóÁ?•Ã£XüZ?î®ZË1ö?"©ÿˆÚÜ9?¥^òpù§?"©ÿˆÚÜ9AGN3FGL J1107.5+0223@o«àe0@Kv 8ðÀ:(¯K²†À;´p'I¿Ë";ϗŠÿ@tRY«î@¿à߃ü¬ìæ¿åá̧ý¤¿çN±Š"±¿¼
-Ux­fAGNbll@žîˆ˒:PowerLawNVSS J110735+022225?ïþ۝þ‹¿?./ì ÀÂÃ?"Fv]\3?./ì ÀÂÃ?ïÞµ¿-ì'?Fsõû?p¥ d:Cs?Fsõû?ïÍŽ¼G?vM!?yt8áCäs?vM!?ïý–1ðÝ?"d#-oï@?3Nw¤'Rà?"d#-oï@?ïý'I´Ã°?<þ™÷ïŒ?6ųÔáo?<þ™÷ïŒ?ï=2wÃÓK?¨ðª)b8ª?˜Y±
õ2?¨ðª)b8ª?ïuþÅÿd`?Ž>M%tD%?'@'>[¦?Ž>M%tD%?ïÏ £}aï?us"ñÎbD?xo®Z87?us"ñÎbDAGN3FGL J1107.8+1502@mIÎ ‰ãC@Oˆa .QÀ9®JGKîìÀ;«å3Ëßg?ч–u*'@"þ¾·`T?ÿÙGŸP覿á
/±|¿àVY/"Þ¿Ó‡Twüeí¿äþw}¶^AGNbll@ V\'ÑNPowerLawRX J1107.7+1502?ïþ¥d¨÷?%YQªrYÁ?%©³Î¿7X?%YQªrYÁ?ïÙK1›rQ?'˜ÿ'ç?sZg(§ïÁ?'˜ÿ'ç?ï㕲6ý?t<5 (à?lîj{#ÚÌ?t<5 (à?ï·£âÀ Ž?dà F[€ó?'W/
]?dà F[€ó?ïö9¿á¤B?X-4*6?SŒ€1¸¼¤?X-4*6?îÙ9nO'¹?¬ Ip"9N?¢liwpl?¬ Ip"9N?ïÊÞÍ<¬?€*½€m…?z™}'?€*½€m…?í¹ú/˜? sÒhJʲ?²0,‡óC? sÒhJʲAGN3FGL J1109.4+2411@jÏu@‰]@P·þ¿ù³À:\ø³¥À;ՎñŸêì¿ëœMÑD*Ò@
œ¯ê"Ý?þ0§á6¼?ÏQ–íå¿æŒâaÖ׿ßÐïì·xÓ¿ ­Ð¬*AGNbll@ª¨Qœàu÷PowerLaw1ES 1106+244?ïÿ["È›Ý?ÚɁxøy?h¾µÂ9?ÚɁxøy?ïäì3¢øF?zw†W,Ò?kÌpEŠ;?zw†W,Ò?ïàíñé'?j»¸HÍv…?oGõ'?j»¸HÍv…?ïÿµVøµ>ö¾½4Ac?¸Û,V"þ>ö¾½4Ac?ïÿ.1IV¿?ȁ"??9ÔWp­O?ȁ"??ïwØÈ>ÙÁ? xùY%hÎ?'æýL1â? xùY%hÎ?ïÈq4ý+?|ŽÐNÔ³?{Çf€ÊS?|ŽÐNÔ³?ïú–	ÓN­?H2H—"y?E§Ù"sù?H2H—"yAGN3FGL J1109.4-4815@qß%¿­)™@&r¬azŠÀ9¥—­[îÀ;z÷Zï:?æbÈ
í Ï@_Kä/@ôÖ ˆ‹ª¿ç8äl?ˆ¿æuºIðí¿ég#™Ñ烿çÌñZAGNbcu@‰`Þ҈ÎPowerLawPMN J1109-4815?ï÷Oƒå—
?UÁÕ(a?Q`÷òÙf?UÁÕ(a?î¬av¬H?±ùï€è?¥9蓃©8?±ùï€è?ï >4ª<æ?zŠaNkÌA?‡ðrË!ò†?zŠaNkÌA?ípӗ—5ç?AãA†Ç«?´ycC´DG?AãA†Ç«?-@?:él­?Õ8¦ñŽ&?:él­?áXvT¬;?ÑV˜ŠrW?ÝOÏV§Š?ÑV˜ŠrW?í—<IÝC½?¥{öï«·
?³F³;£'?¥{öï«·
?Û
ÈÊ"'@?·¦üîz?âyšî¶à?·¦üîzMIXED3FGL J1109.6+3734@fµ'Ì÷@P>àŸ°À:ٟâˆö´À;íܜM©?ىƒ•þ@
ËØ:&—?ú^Çá?â
¶?äê?ïø̜§h¿ÌŽCE鳿̸@	¹ŒAGNbll@¿Å˟U›=PowerLawNVSS J110938+373609?ïýö7K¾?4.á֞¦Ð?0NGæ6»?4.á֞¦Ð?ïÙ
ô¶ÜÝ?k¶(8âÙ?sz…§QA¬?k¶(8âÙ?ï|¹…X€0?Œ±Ã·hS?hÏS8,?Œ±Ã·hS?ï:þ®œ5?sJæ!—]_?ˆ±@TXòµ?sJæ!—]_?ïø«Bl®?P<ØO|æ?MSú¢½-?P<ØO|æ?îÈ˓ð?÷?¬_*‰ »?£sFÀüŽ?¬_*‰ »?ïcåÕSÑ[?'%8ñ#ž?"ƒEN¦œ°?'%8ñ#ž?î[²Ÿ?£N#à–Ž?¯NZAo*?£N#à–ŽAGN3FGL J1110.0+7134@`µJ`"@E°…ߨq¤À:P­'tâ*À<î
46h?â¸D{"@ƒ`ݐio@>îÿ|¢h¿ã5~VƒV¿ä¿ß"ƒ7á¿Ñú,›-\¿äDŠã76AGNbll@¦Ž>«6zPowerLawRX J1110.5+7133?ïþŠ™Êl?@^Õ=¾?'^™ÙŽ"?@^Õ=¾?ïż¸¶?ˆ%¹h?}!£˜'ßÉ?ˆ%¹h?ï¾R#õcÖ?…v¹œÕt?€kvþßx‡?…v¹œÕt?ïfÔ³©˜É?snʦhrM?"%i'5àô?snʦhrM?ïøÛÞãz¹?SOàg²4|?L…?°í[?SOàg²4|?í¿ºï:ò?·À´±M?²(…L‰?·À´±M?ï'Hêîv?'¸ºÖ?mû"6w?'¸ºÖ?ì'«>¡j7?¨Gït?ãˆ?¾Â¦
ô®F?¨Gït?ãˆAGN3FGL J1110.4-1835@q6_Ø­¬@CȾâ(À9Pc¥ÁÆ	À;uéÀ"š_?å'ÎÕÌ@x^áaÚ@)? ~æ?žÞ¤Kàdj¿ãzuNX¿Þ¦¤*Ru)¿Þ÷Aö¢>AGNbll@›4†Â&€PowerLawCRATES J1110-1835?ïû
Ðñþ?@î.çÐsæ?CÔ¼‰ñ™£?@î.çÐsæ?ïÁôȃ+?‰@%á›N?u…"a²?‰@%á›N?ïÒÖm¤7?ue3¯Æü?v"ÉH±f>?ue3¯Æü?ïq 6æœ?m>qº3k]?'Ëù=C,{?m>qº3k]?ïõ³T'ä?QùCuè
í?Tz™"Ȩ?QùCuè
í?îNoàÉÀ?°sÝÙB/?«ï|#?°sÝÙB/?ï'1/Ó|?‹«oš?‹³´1|M#?‹«oš?ìUo‡™´?¢ºÞÈ(Ìs?½W¼ƒÃ2^?¢ºÞÈ(ÌsAGN3FGL J1111.9-6058@r2iŸ¡—¿Ù<ޟªw/À7æ>)0zòÀ9ôúWI'ñ?ú…aêhi@0{âN"8?ü}¶¬¤ä&?ïÿ‡¨3¿áÈ%Qâ傿å<"Qw°ª¿êý~ñL³ãPSRPSR@®q§E8ï5PLExpCutoffPSR J1112-6103?ÀäŽ)ÎÛp?Ê0Àì]¥'?ëÆÜuŒI$?Ê0Àì]¥'?ԑZãGÚ×?Éì×·¿þ?å·RŽ\"?Éì×·¿þ?Ïã<møÃ?µjhœ</]?è0äýÏ?µjhœ</]?â";^®i¾?±Ïx˜4Ï?Ú׉B£,"?±Ïx˜4Ï?š|‰cLÁ?¶'IÛkK(?ï,´¼_Â?¶'IÛkK(?¸_¹ Ž"?¼kõ‹K¼Ü?ìôÜ%7û?¼kõ‹K¼Ü?¿` ^ÎÒ?»°XUŠ(Á?ìûô=æ&?»°XUŠ(Á?П85aÇ×?¶&4pj¹?ç°cåO?¶&4pj¹MIXED3FGL J1111.9-6038@r0Žàm"¿¶nŸËùÀ74éœlÀ:Í<^U @Veòùg@¿lÛËmQ?û'ýXZßõ¿àÍD@÷–û¿àŸ|Ò¹uØ¿ã@Pó7š¡¿èŒZ{v™OTHERspp@§F;¥ãSøLogParabola?"ï(CwZ?"¥©Þbœ?ï¬C_½r?"¥©Þbœ?¤{Ñ2'Bp?¿'õ::u?î¸BìäšI?¿'õ::u?ÓVCEF}Š?µZæ,¼˜ï?æTÞ]\Á;?µZæ,¼˜ï?­ Dôõ·‡?ŽyK#˜E?î%û°Ì!g?ŽyK#˜E?Šñ'x~'?‹žMBà?ï¹Ô;oÜv?‹žMBà?Ši{/%{r?ªîïFC?ï–Z5«¢?ªîïFC?Ó¯ž«–
?·C(®%ëî?æ(r°ª4û?·C(®%ëî?€TPyìq?n®"²¶±ç?ï¾®¾ÑÊ?n®"²¶±çPSR3FGL J1112.4+3449@gZã`'@Pàg@™ÅÀ8ðùÏ5]À;­Ôèë?ôÉ5M¿¦t@v˜¼¤áv@Á»=iè¿Ü €±žÒ¿æ·¶Õê'À¿éÇRºb¿ç6–ŒkU0AGNfsrq@{W5?|í'LogParabolaTXS 1109+350?ïþÉܼ(?#@â¡n?#cÄ1«;€?#@â¡n?ïÎâÕ]ü?G"WU:f?xðŽ•Qó?G"WU:f?ïœá¡‰ìÂ?ƒ-1VY;ý?ˆÇ—"5û…?ƒ-1VY;ý?îúhÃÛ.?{C«
c;? YsÄíŸ?{C«
c;?ïýÐ2æd×?/¯luóÉ?1~hq–Ûó?/¯luóÉ?î·r`MPH?ªùJY?Œ]?¤ˆÙû*ûy?ªùJY?Œ]?ïbGHæ?'#IpÆÃ?"¼—o_7?'#IpÆÃ?ê–hˁ¯S?°N/xn?Ŧ\ÑùB³?°N/xnAGN3FGL J1112.6+1749@l¿VÀÖõE@PZßÎ1QÀ:×ï¤h)µÀ;Òÿ¬óéq?âº_ð*Ÿç@ó×QÑ?÷x‰ ¥'õ¿í-?ö‡~¿àåñ!ö¿Í`E|®HË¿³"‹RYBAGNbll@ËPá©ûçmPowerLaw1RXS J111224.2+175131?ï3áu.?Âüa/Dç?™œ#ց¨ø?Âüa/Dç?ïàÉ!FL?€Zú45¨?o6ôµ~dz?€Zú45¨?ïw&÷l¶?'ñBFâÃ?'!Z›3?'ñBFâÃ?ïã¦jYÝc?YôC—¼Å?lY•êÚÌ6?YôC—¼Å?ïùÐË_?R%wƦ'&?Kˆ¼ÿ''?R%wƦ'&?îÛÍó	ð?¯¢v¡—ËÖ?¢NƒÞ
?¯¢v¡—ËÖ?ï}"¸j+?Ž§du"î:?M‰Qò‡?Ž§du"î:?ï'
.p?•îfeê´w?œo¾Ušú?•îfeê´wAGN3FGL J1117.0+2014@l2؈v\@P×°`À8œnØû¯8À;"pdìêÀi·|¯Þ@=oxˆÒÍ?ýÝÎg¿Ø£f^P9Ì¿Ý,éo<EM¿Û•7	V•ä¿ÚžoP^«÷AGNbll@ _Iûçl‹PowerLawRBS 0958?ïÿ»-Ý)>ùaSڇe?4Ÿ~'ŒŒ>ùaSڇe?ïÞ@%\?…¼X8åʁ?pßñtNiñ?…¼X8åʁ?ïáò©*[H?qÕì¤;?n
V´¨wÞ?qÕì¤;?ïÿÿp§Ì§>ÁCW>'ìiãV>ÁCW?ïÿ…€ÕIë?
|n]"?ŸËAKgè?
|n]"?ïv(G¿(Â?£Z"r©šâ?':÷«KÎ?£Z"r©šâ?ïçñó;»1?z—YÆknï?h‹ë7q?z—YÆknï?ïÿóNQ$>ãf†ÖNî>ÙõHÒèÝ*>ãf†ÖNîAGN3FGL J1117.3+2546@jgžÿŸ‡ð@Q:þßÙïËÀ:']æe$GÀ<
µùK°Ø¿ä…–À l@
]zž,@,Ù¿úVs¿é&•‹Bõ¿ÃÑ9æM¿å(©òçz¿êaÃ$#îAGNbll@%)ᰉ PowerLawRX J1117.6+2548?bɬe?‰ö65m¶l?‡ß§Fµ®ê?‰ö65m¶l?ïÜ÷®3æ?…Šøß'×Û?q"(úcH¦?…Šøß'×Û?îBÜ¿;È6?›hšÊÑ\ð?«Ò4³Ÿ?›hšÊÑ\ð?ïóÔ,4?F‰Kã
x?YðWÛÑÿê?F‰Kã
x?ïD¶Gœ™ ?"Zêc3÷–?—i7lÜ?"Zêc3÷–?ïD젟Î?©4–è?—bkè­ê9?©4–è?ì<÷Y_º?«Um‰Š¼?¾E5/?«Um‰Š¼?¿ï?œãMËB'©?¤EäoÕ?œãMËB'©AGN3FGL J1117.7-4632@qéî@…+N@*¯a	/TÀ9…oîMPÀ;tÿ^Ë?õ{ât(ñ¼@ÁQ&
ZÜ@qA%iǿѱg
üx¿ë2ÉlCÉ¿è…î)qq¿ÖÏ,;OêØAGNfsrq@Šžcø¶PowerLawPKS 1116-46?ï'òƒô~?ÝvŽÝH?‹C_
G4t?ÝvŽÝH?î7@ë-?²á
X‰ß?¬‹ÿŠá±;?²á
X‰ß?î'Òڃ?˜Z™ÿp
?¦ßþ"Š%Ï?˜Z™ÿp
?íÞynşK?"gåf¶š?±4‹ŠÓ§?"gåf¶š?ïbfýe?£µùSk÷p?œ³³t$¨?£µùSk÷p?á­°5x˜ÿ?Ò¿(dM1Œ?ܤŸ•Î?Ò¿(dM1Œ?ìß]Ýùq?¤òEÌû·??¹¥gú?¤òEÌû·??ä"9t"¦?Á«âãJÎÁ?Ö׍ö³ó?Á«âãJÎÁAGN3FGL J1117.9+5355@b¦²_c<æ@MÑ?ùSÀ9ŠKn"['À;µ?Cä?èY²òÂ;
@¾Æ/ú™?þâà?Ee:¿ãTö0À´ˆ¿Û¹Ò;C}¿Ü|¸¦²Ì¿ÜdŽ="¨ÕAGNbll@ Ñ·škP±PowerLawNVSS J111757+535553?ïýî$á5å?*4Í5N"?0ŽÚâ¦J?*4Í5N"?ïÏk¦(|?"	Ζîœë?xJv±»6?"	Ζîœë?ïß.û&b¦?pԼȯD?ph'Š[Pš?pԼȯD?ï<âiA7-?vñ~…ˆ"à?˜c²Ðùâm?vñ~…ˆ"à?ï÷N=z´Ò?M¶yõòF?Qc…Ô+Ý?M¶yõòF?îK+ðHÒØ?°˜0ÔÅOç?«M@ø߉?°˜0ÔÅOç?ï¤Ä¾N?‡9ƒPÏGÉ?†Îÿß@]?‡9ƒPÏGÉ?ꨡ;úW?¯¹<¬l?Å]{£†?¯¹<¬lAGN3FGL J1118.2-0411@p{1\1@I·ª RÀ93_?*¸:À;ˆüàÎð?ò_9ßÞè@™+û[€"@…è j¿ã1Ró9j|¿é–žN¸ä¿è_x՘'!¿ïølD"@AGNagn@Þ¼¾aÏÿPowerLawPMN J1118-0413?ïùSEÛ;?DÞkf'0ÿ?J²ëü«?DÞkf'0ÿ?ïÓÕµK?‰Û'_Jš?v•A‡=-?‰Û'_Jš?ï_5Hûá&?ƒÛœ|W©\?"VÛ\q@?ƒÛœ|W©\?ïèû­'Q?Mû>È X?gp}Ö¥?Mû>È X?ïý	bvº?8ÖÌu¸3?7´îRAá?8ÖÌu¸3?ï'&á@L?¬AÉE{+½?œo»#×öw?¬AÉE{+½?ïTüå!
?–É:iÈ­?µ`j;³?–É:iÈ­?ï±wdnF?wf´bÈJ?ƒ¢&×Â`™?wf´bÈJAGN3FGL J1119.1-6127@rBTߋr¿áVnßå6À70ˆzdØÀ:I=tՔò?ꦥ3‰Lù@ŽzóXh@ßÆ´{G¿Ý"û10›÷¿å-æ‹Ý¿åÆFª0¿è–Ý
Bà6PSRPSR@'»˜ÇãPowerLawPSR J1119-6127?êóõÏG¦?ƨVéÏDª?Ä0+ìÂág?ƨVéÏDª?ì©
Õ֋½?½˜yôb½å?º·'QK¢?½˜yôb½å?æõÅ.rÚ?·œü3Cƒ ?Òu£KÜ?·œü3Cƒ ?ë~×!ÅÍ?¡'5. ~ð?£³xèÊ?¡'5. ~ð?à¢õì^?Ñ1+¤§m?ßûüº'C?Ñ1+¤§m?Ù
ÏïÆU?Îm#ºkâ?ãy{ˆÖ?Îm#ºkâ?âȹώã?»n?RÙt?ÚnÔ`â:?»n?RÙt?Ø6è9?ºÎK´Ö®D?ãä‹úcw¸?ºÎK´Ö®DMIXED3FGL J1119.7-3046@qŠA [À@<J€VÒuÀ:¼*JVegÀ;ÔËÔI¿×)»9t@"e²â?ü?ø¡, qúï?ÕQ{ˆ6šÇ¿è3Ñ\î1e?é
bh™¶9¿Ï€Œí¹¬_AGNbll@ÄÛQ&éxÕPowerLaw1RXS J111941.0-304652?ïþý
¤–?BfٙÇ? /Sëîu?BfٙÇ?ïâ7ÁsŽ~?u¨
:ãv?mÈ>»,1{?u¨
:ãv?ïÚÊE«RK?r•Rni?ršÝ$×zy?r•Rni?ïÿ|·áƒ=?§YZfï?i"=¤®?§YZfï?ïþT=ç8«?+²É8·Z"?*¼¿ê?+²É8·Z"?ï
–B»Ö?´üo×È6?ž­7£]Ò>?´üo×È6?ïжf?5?y;)Þu?wô$´Ó!t?y;)Þu?ïþük17—?%_µnª? 9O¹hDš?%_µnªAGN3FGL J1120.8+4212@dúë__(@PŠ¿Ý/ñÀ8Ç¿ÝÑÀ;øãú?ÖNL¿ g@ÿyZ3þ	?ùܒÉ仿â_qü¶cC¿Ôô¬'Ýóï¿ÎÃÕÍ|u¿ÇG¶Üå7—AGNbll@°Øõ\PowerLawRBS 0970?ïñ£.ÔåÜ?a÷É1Œ?\¹¢^sW­?a÷É1Œ?ïÚ	ƒ·Z?‡@²ãò¢,?rû>@¼l?‡@²ãò¢,?ïQ_Ìqç?p*PÐ$?•Ô€a_"?p*PÐ$?ïÉKٔ©?dWé}—}?{vYùȏÆ?dWé}—}?﹌9V/?€iy<î"&?¿ÜûùH?€iy<î"&?ïÒXÛl?¤çÅ¢Ë?œ´æJN?¤çÅ¢Ë?ïœõf€?–#°Dû?ÌaZ‡ô?–#°Dû?îRßVDã½?žƽ@?ªÒ
œ«)?žƽ@AGN3FGL J1121.4-0554@p£Â # –@I9PßìdBÀ8H]®îÀ;NO~ÃT~?ñ¶O)Þ˨@ÌápGæŸ@î"ßu›ã¿à±`²iÁ‡¿æ'þ'o¿ãÀ¥«ºrF¿ìd{йtAGNfsrq@‡¦ŸŠ	ÞPowerLawPKS 1118-05?ïòíÊb(-?l'	'Rf?Z$k¿ ¥6?l'	'Rf?ïÖÄTG³?†wkÀo%»?tòõxŽ?†wkÀo%»?î܅L/®n?"ó0éËÃà?¢7«=á?"ó0éËÃà?ïý°òsù?gÌfD?2xn>d	?gÌfD?ïì±›Ã.?iiíÄfc?cNð`I®?iiíÄfc?ï-fï36?°7ÖÝ9/
?šS"EÇ.?°7ÖÝ9/
?î>_)cÚ#?žgˆhPc?¬
evÚÛ?žgˆhPc?ïüN†ºˆ–?8HM݉y?=‹ËŠyÑÑ?8HM݉yAGN3FGL J1123.2-6415@rX'ßüTzÀA¯ó£À8\š1o
ÕÀ:áN_¤?ø&»˜Çâ'@g?A‰b?@å¿ÚËè÷¿ä[[¸ã`ã¿êŒ#0J_¿ëd—iò¸¿áHê¥êzAGNbcu@u5¼ýKð™LogParabolaAT20G J112319-641735?ïý?N}9?6ð›<"?6Ž¯	?6ð›<"?ï.¢.,|ú?«Æœ<NIk?š+º5Höº?«Æœ<NIk?ïX:Ú?"ÝÈä ü?ßtöö6Á?"ÝÈä ü?ïXJnä?rœÉ?Œ)í]gÄr?rœÉ?ïõ¸m3#?YFõEÒ,?T%s>R?YFõEÒ,?ê&È&
Ë?ÇÅþ@Q¹?ÇfßgÈÖ?ÇÅþ@Q¹?îRÚìtÞ? [æän'?ªÒ^,í/)? [æän'?î<]â;ýe?¡"Føs)ÿ?¬:!Ù¬t·?¡"Føs)ÿAGN3FGL J1123.6+7231@`xÀ Ç@EˆßÊÖSÀ; ýŠúaÀ<*%@+i:?ñ_ &P¡®@	†ÁEA?ù~sÝ@
¿ì'‹'nŒƒ¿â ×@n¿á^ȓy'?Á.å»Ü´AGNbll@ɧ›Æ§ïžPowerLawRX J1123.8+7230?îº\ãŽbâ?¸2Ok·®ä?¤Z1ÈџØ?¸2Ok·®ä?îKõz°ô?À¶‹í´xî?«@¨`¸¥Ä?À¶‹í´xî?í܍n+ñd?¢âOÌ;??±"êO\?¢âOÌ;??îãqf—?"éÔNa?¡ÏèçÞÁ¯?"éÔNa?íô|ç\E%?¹Z	ñ?°\ÃÓüW?¹Z	ñ?âxѬŸI¡?Ô§ÙxVÓÌ?Û\¦Ál¿?Ô§ÙxVÓÌ?ëœY¾k?°ƒ¾Óõ<?Áž™ÎV?°ƒ¾Óõ<?åØ;¯UÖ?É¡²[¡*?ÔOˆ ÅTU?É¡²[¡*AGN3FGL J1123.9-3653@qÁY_í¦a@6Â<à[À9
´br»ßÀ;Œ[™ƒÊ$?ÿ>åCJü@X°få'A?úšÚ\ˆ–¿Ñ ˜Å'οÜëYοáZŒÿ_úš¿íZå˜ÞPSRPSR@•g	ÞÒPLExpCutoffPSR J1124-3653?-•4ÐÒn,?9K$¤\3?ïþ&¬Å£ì?9K$¤\3?±LG2¯ÚÃ?»ëøŠ{]?íÖw€ÉX?»ëøŠ{]?°D2ÙÍåq?Ÿ¸'I&+ç?í÷y¤I'?Ÿ¸'I&+ç?œÂ'©hÙ-?}Ÿ.¥K%Þ?ïëj‹}ç?}Ÿ.¥K%Þ?LØcn8fª?@¨n6H?ïøÉæú†«?@¨n6H? Y&Õhj?²)[ƒ‰aé?îúm'æ³9?²)[ƒ‰aé?"™²Þ?Œæeð·È
?ï[7G®¯?Œæeð·È
?e>± /bª?Ruî
¶oš?ïêÁN‹Ë?Ruî
¶ošPSR3FGL J1124.1+2337@kDÛ@-¹@Q€%ߙXÀ9ºJ«õ¼°À;ÛjÕ`ð¿ö9ühEä'@W©¯¼EÁ@¬=?üoR¿å(þ§Ê¿è‰.+PU¿ßžo¸…Ô&¿ê®ûC€AGNfsrq@…ºÌ~($PowerLawOM 235?ïý›Eã†o?/N`¡¨Äl?3%ÎÜÔW?/N`¡¨Äl?ïâ§Ñ¯yo?ƒ
'Ã%Gý?mX.3©Ù?ƒ
'Ã%Gý?ïÆ~:Ý:r?u£ 'Ð?|À⌓S?u£ 'Ð?ïÿˆs¬u?œ‰B_•?
ã÷$¶?œ‰B_•?ïþO¨M«H?+O‹ÿD"?+x\ϱH?+O‹ÿD"?G#)? é!mî-
?\îèa¸? é!mî-
?ï¼crˆŒ?')QqZ‹?€ç#eäÏ?')QqZ‹?ïõ0åaTj?Sï7(µÔ¬?Už5E–<	?Sï7(µÔ¬AGN3FGL J1124.5-5915@r@@ Ç?ü5:ßÏÞÐÀ7ƒ¸µ¾"NÀ:|{üР—@&,§¨Ðï@¨Ù>Ú[@ƚŽ½¿ßل ä¶¿ã}á·aøæ¿é[J÷š¿ëet®/PSRPSR@Ž­k@öjUPLExpCutoffPSR J1124-5916?C~÷+ß]?ISntÍ?ïû BsJ®?ISntÍ?¡ÇÕNù?¾XË1Ô?îî(K±Q?¾XË1Ô?Èš5….?²,5šA~?éøY~²ž´?²,5šA~?'ÕVûæž?i~|.eZ?ï´ª£úh?i~|.eZ?;'¹¥ÔË\?8¶ù¿ªã¯?ïü¨ÝŒì?8¶ù¿ªã¯?ŒÚògVŸ?¯C%-Øâ?"_õ?¯C%-Øâ?™&34#?•²v³†AÝ?ï7Ö΃[??•²v³†AÝ?H;ôº l?<TgßÉS]?ïùñꞢ?<TgßÉS]PSR3FGL J1124.9+4932@c4ú D®†@O /µÐÀ:dpA±{8À;탠Uu¿Õ.Bç
ô=@pG´Iž/?üل`wd¿êÛÆwž5¿Ü‹æ¨b'¿Ó›'Uy¿ÃžN¬'ÍAGNbll@°´9‡+PowerLawGB6 J1124+4933?ïÿŠ+èf0?GÛ¬Ó£ý?
uJî-?GÛ¬Ó£ý?ïç¯h¸?xDóýL?hPúÕ•?xDóýL?ïß©+e'	?z'ûQèÔ?p+j8™SÃ?z'ûQèÔ?ïÿjAÎg¾?|ˆi3E?·Í@ÞÉ?|ˆi3E?ïÿi{³nq?
%ɸ*?Їƒ¿°¡?
%ɸ*?ïl±°€€?™ob`ׯ?'|IÐÏ(?™ob`ׯ?ïÊD#gÛ~?ÁÒ¶Ž?zÝîdÏpí?ÁÒ¶Ž?ïû
c&&A?=çÈÊoó
?CÊsàY<ù?=çÈÊoó
AGN3FGL J1125.0-2101@qT%à.©a@BÀy`>.9À9øŠ(Ž"À;"ýs]Å®¿'½É;²Y@
÷áíEh??üŒ»à@r¿ï`ó˜ÇZ?é<Õõ"@¿â8Îò'5Š¿ÆÿxñƒeAGNbcu@±¥ø"t¼jPowerLawPMN J1125-2100?ïý"›J?BKâË.&=?3g>St'Ý?BKâË.&=?ïÔ_¡-ë(?‡;dêlC@?uÐ/‡öç¥?‡;dêlC@?ïÚÈ)
Kš?sýaZç?r›ëxƒ8?sýaZç?ïò¦aíʍ?HæÅÊîcÈ?Z³;çñÆ?HæÅÊîcÈ?ïù¤û2Ìí?J×JK ì?Il0ó"?J×JK ì?îòÜÛ°î?³^+Â!? Ò2G'ö?³^+Â!?ïÉx8Ã7o?|-2Ðþ-ð?{Cã¶qŒL?|-2Ðþ-ð?ïX:CI0?Œ¥b¯G?"ø·–—¢?Œ¥b¯GAGN3FGL J1125.3-5824@r=y?ò^W@Î0àµÃÀ8ôËá©ÔÀ:§TÚLè?ñ¬·xÒ¤¨@
ÆG²œ@‡_ZX'?í´…hñ¿æ[›l-¿ßìÅÇ¿íV" ÞÇÌPSRPSR@'Iº^PowerLawPSR J1125-5825?Àۖǵ¿H?ÄÛM¿Ñg?ëÉN.?ÄÛM¿Ñg?ÛÙÁZ†g?Î\Á	}µÁ?â|R¼Í?Î\Á	}µÁ?â³XÏqd>?³T|˜9ij?ڙNa7…?³T|˜9ij?夥»½ ?¯à·úÁ?Ô¶µÖˆ"Á?¯à·úÁ?ª=T¬!(?·	î«VËã?î\*´ù5O?·	î«VËã?¸
ÞYÏð'?½É,!yªï?ìþD4üû­?½É,!yªï?Ñò‹‹—€î?·7F9s‰Ó?çº:4?‰?·7F9s‰Ó?Ò"¢`cÝ?³RWj
ÿŒ?æî®Ï¿N?³RWj
ÿŒMIXED3FGL J1125.5-3558@qÀ» 1ί@7»'ÿùJÀ9LPtTfÀ;ZHþv"?Óɯ
@§²@h"qM?þ"tÿ±Pš¿Â¦¹r|õ¿Ú·µìêD¿ÚÈoT†¿ÙZÝsZAGNbll@¨#É7KƨPowerLawPMN J1125-3556?ïþÊþÒ{? H[­•Š?#^ÜlB—? H[­•Š?ï҈QXôI?….Iãz˜Š?v»×EÇk?….Iãz˜Š?ïܶK£cê?r@<‡ z?q¤Ú šý?r@<‡ z?ïõ¬S6f?7¾RCÂq?T§ÑC•³0?7¾RCÂq?ïý"äl·Ê?7l0?ÕEÄ?6èÝð4dT?7l0?ÕEÄ?îý ë® x?²Bü›Dà? %ñC^*?²Bü›Dà?ïÛ9&A³?|*!y:ì?rcsVᦊ?|*!y:ì?ïÇ4P®]?j(ùYVã.?|e×¹O˜u?j(ùYVã.AGN3FGL J1125.6-6012@rG[€#¦Î?ìû8ÀcïÀ9*]ÔÏÀ:²Qaòc_?î%%‹ç@ö%ÍD@ýÔ¿_{ç¿Ãîü'Ob¿æ̑'§†9¿èT–cjnÅ¿ä25w08,PSRpsr@ $ó¶E¡ËPowerLawPSR J1125-6014?ï4	èA¨?£Täö_#?™~Ã.Ñ?£Täö_#?í­lÈí?¾ŠB°öúÀ?²—, g¬?¾ŠB°öúÀ?í¶¹ÉÿÅ?¡úôIÚ?²J1°qåZ?¡úôIÚ?íؖp*››?‹"Õý{6?±;Lôý¤?‹"Õý{6?뀒5"ë?Äû‰xº&?Áý·+áìU?Äû‰xº&?ÞVþÆçR?ÏðÌ9ºb?àԀœŒW?ÏðÌ9ºb?çI\5Çr?·~‹ìÊÓ?ÑmG"qÅ?·~‹ìÊÓ?ãæÑÌ¢Ð?·g3»7[Þ?Ø2\f»Ô`?·g3»7[ÞMIXED3FGL J1125.8-0745@pÒäÿÉy[@H·&_æ¥À:oæÃ%À;ÎCG}m?'É£a>jf@ˆÚY¨=?ÿB*Z~&¿ç­¨,·÷†?ÒwF™¨™M¿äÉns{"¿ÙªaµEAGNbll@©˜~BZîcPowerLaw1RXS J112551.6-074219?ïý€ô(¨¸?4¶˜Ÿ,•?3ø][ûºñ?4¶˜Ÿ,•?ïØ3ïàf÷?'×Ê,ß\?sæòï̃?'×Ê,ß\?ïÏ*ó?rBº#Ï«`?xj·¾¦¤?rBº#Ï«`?ïê 52D~?Ožq¿u°?eßÊÿ5áT?Ožq¿u°?ïöؽ#•?UŽ*zOðå?SÒN0'†Z?UŽ*zOðå?îîé›uÍô?±IKe?¡fFëRÈ?±IKe?ï™ò^EŸ`?†.ÙN"Ët?‰ƒhg¸ïø?†.ÙN"Ët?îÑô£oJ?—ëó¥öì}?£Æà¹8§Y?—ëó¥öì}AGN3FGL J1125.9+2007@l`xÜ@QO?Ï"èÀ:k™èsòÀ;÷úŠu9h?Þ[g/ö#@'ð=?Q@}?pÙ1¿yt]þkˆî¿ç	Ž8f¿Ûš+5Ÿy¿ïÿÎÍ&ÌAGNfsrq@'ÔÒ×süPowerLaw4C +20.25?ïù
mõ¯x?Wku®Á?KÖGOXÖ?Wku®Á?ïË«So,¢?€®HëŽ?z*V:«>á?€®HëŽ?îMŸge¯?šD´8LÜ?«&­¾?šD´8LÜ?îðùq	q]?ƒ9–Vû? ðhò؆1?ƒ9–Vû?ïùÉ×\{?Vëa±Ù&?HÛÍ4Ê>‡?Vëa±Ù&?î9ä	³?´1ÞßÍD?¯Œf&
çÌ?´1ÞßÍD?íÃ7Qݜ?¡×0Üth?±æEv…,?¡×0Üth?è|ñRñ?·nD¤ßBÒ?Î:´9‹›?·nD¤ßBÒAGN3FGL J1126.7-3834@qÔ_'`@5aTÿ5Õ¥À9üËE%¤À;µïXz?Ü{Fþþ3ˆ@ým"V_@)_ÊÀÙ¿¨Wx6ó\.¿ãü狃Æ
¿é¢<a@ró¿ÎìAÁ/N'AGNbcu@"à%+ÓÃaPowerLawPKS 1124-382?ïó…LŒ?f5/}ƒ?YÄõ§/Y?f5/}ƒ?ïÃWEa3!?Œ¤ÙEân?~T]d"?Œ¤ÙEân?ït»ëº4?"Í/lUóå?'~(}aO‡?"Í/lUóå?ïÐÒ(^÷e?a¾A؉6Õ?w–ë葑r?a¾A؉6Õ?ïxKOM‰å?œÀ$5>{?ö––õV?œÀ$5>{?îOÂ;?µjan|?«ÜM[C?µjan|?í£M¢u5a?§è֖ð´î?²å'î"ô?§è֖ð´î?ímF/9T?©ðX†;?´—¥Ð«öá?©ðX†;AGN3FGL J1127.0-1857@qK…ߨq¤@Cʉ€Fâ=À7R_IÀ:æ3hXÔ?øbýPMJa@ð"gXSÔ@/8Ç¢¿àD¹¦h¿ä@W¡&«»¿åC¬':׿æ¥N…ÁlêAGNfsrq@y×m|o½'LogParabolaPKS 1124-186?ïýD}À§?52N=Qh?5Üö¹ T?52N=Qh?ïЊDù?Š')VéÛK?wºÝvg4G?Š')VéÛK?ï¦5?85b?ƒjuÃgO›?†r°$47¡?ƒjuÃgO›?ïüj·ž?-†Ëõ(??ÏܔE'Ë?-†Ëõ(?ïú¡"¨#~?Dn¯…Œˆ\?EyíÂó…R?Dn¯…Œˆ\?ï9øT˜':?§ý…;é'?˜ÀõlíØÐ?§ý…;é'?ï€%ª3š·?âAÎãoª?ö•}h&(?âAÎãoª?ïú´ÏUV?Bã˂¬æ?E,ÂÙWÝÃ?Bã˂¬æAGN3FGL J1127.8+3618@f‹-ÿ'+¿@Qƒw`MÉÀ97¢ô§À;¢1¿•¬¥?å,>>v±@"¡Ì@Ë;\_¿Ùúö~ªˆˆ¿ç+Q í²¿åœšQÇÀ@¿ã3÷ã?Ä«AGNfsrq@Ÿìô!-PowerLawMG2 J112758+3620?ïÿ­9´§?¦é·ÎŸ?±£æî$÷?¦é·ÎŸ?ï傠٩Õ?{ÂgÚ›?j}_#–{	?{ÂgÚ›?ïÑ Ús²?u,ÒNŸ}è?wo'åxT?u,ÒNŸ}è?ïø& td?2ú»áÉË?Og€ڄ›?2ú»áÉË?ïÿLñ A?SÎ>!¾&?¬Âü>ð?SÎ>!¾&?ïs¶èMË?¡WÆ̓Ó?'‰"öF*?¡WÆ̓Ó?ï^ÝlÆì}?'Mž‹ŸD¤?"$R`C8n?'Mž‹ŸD¤?ïÚôÒǯú?eºCY-Z7?r…–¸TÎñ?eºCY-Z7AGN3FGL J1128.0+5921@a§É`0Â@@K[€"ØÀ:hJÆͯKÀ;úÚa
¿é†ƒÛÓa"@
Õ´¿%D@¿¼w¯d¿æÜkûõ.¿æóý¤lA®¿ìzmôWß¿ïÿK'$°AGNfsrq@':^J82PowerLawTXS 1125+596?ï÷ëv.?Pä@݀Œ?P(ߊ'ïÎ?Pä@݀Œ?ïß̓ŷ?ƒ—OåŠü¥?p~WŠ@Ž?ƒ—OåŠü¥?îì`œ*¡?ß£¬&•ê?¡9ö?é£=?ß£¬&•ê?ïñ6+¾¨O?N—‡$Ö?]"¨a³!I?N—‡$Ö?ï÷¶æI?Q½œÊMÛô?P'2áÃmÂ?Q½œÊMÛô?ï07×Cœ?ŸˆÐþȍò?™ù†Œ?ŸˆÐþȍò?/'h'?›ÆU(?S?¦•½­Ü?›ÆU(?S?íÞ"¹&—?¨"º<Ëd!?±	ëÚ¤¾Ë?¨"º<Ëd!AGN3FGL J1129.0+3705@f>A [À@Q~³Œ¼À:Rîº]À;ÁXù–Ys?Ö!¥Z@8É˳@¨Yÿа1¿æ^µÀ@ÍP¿ãp«ëº¿Ü(•kÈ·%¿åÌÔkÉôùAGNbll@¥YÛ"ÐåPowerLawMG2 J112910+3702?ïÿëgíz>àx3·>ä—øöR£Ÿ>àx3·?ïè+va—[?wïBÖìw?gԉhνi?wïBÖìw?ïóì¡Üç«?g|Æ×ï°r?X&»Äÿ[e?g|Æ×ï°r?ïó2"?>Ê1t¾¯-?Yñšâÿ'?>Ê1t¾¯-?ïÿâDÇôæ>ðâˆÍY->í»q7ÍZ_>ðâˆÍY-?ïj8@õNÝ?•Áւ5Ø]?'¸÷æ}ŽP?•Áւ5Ø]?ïñßýðÊó?oúKEÛ?\@ª÷;i?oúKEÛ?ï¬+vÈ«¢?uê+£a	€?"õ"["‡X?uê+£a	€AGN3FGL J1129.4-4215@qñÂà°«@2nÀ§û\À:ŠÉòý¹À;¿IÍ©kŸ?ޞÏà
Øl@U¸™9@ݵ_Ƚt¿ê<âcâÓt¿ÖAéV<Äú¿æ/–àÏ­¿ïÿìã~Ñ(AGNbcu@…¿oÂej¾PowerLawSUMSS J113006-421441?턌» 
M?¹èÙ2`ÐO?³Ûš&#®›?¹èÙ2`ÐO?Ê]'?Œ	†W½?‹aÝ'©?Œ	†W½?ëCÄüÚí³?¬µá¨öK?Âðì"I4?¬µá¨öK?ì/ò?"5q`É?§5Q<$÷Æ?"5q`É?쟧5õ—?ÀCÃjò+?¿£ÆPSL?ÀCÃjò+?êŵ±¨.2?ÄûÌ(I˜?Äé)9_G8?ÄûÌ(I˜?èqÀ‹I†?·Dwý]Px?Î8ÿÁÒÙè?·Dwý]Px?ä¸"@?´âmµõv¸?××ÀŽÙÁ?´âmµõv¸AGN3FGL J1129.9-1446@q3nÀrKw@EÕñŸêìsÀ8¤˜ÒÊ<ÐÀ;•¯,¨Õw?èãà:5@õ`ªåœR@Kà˜†Ÿ¿è.&Ãۃì¿èTB齿ìUÂõ]¨¿ïÿÆւqúAGNfsrq@tñ^Ý)5PowerLawPKS 1127-14?ïþ‹Òî$?$¢E¾2ç?'OÕi8¢%?$¢E¾2ç?ïÚÖæ+B¤?•¬p5?r"Œøø?•¬p5?ï'TöýLò?±Gq?jÂ2îS€?±Gq?ïåºÅõSe?Pe·°Tí?jE9ú.{/?Pe·°Tí?ïþL?1ó#|t?+?ðƒ6m™?1ó#|t?ïe&u_©?°ٞéÐï?œÓ[*tÒù?°ٞéÐï?ïH¹QgH0?'ñF´j\?–èÕÙö1ô?'ñF´j\?ïg59%n,?…È{½PË?"XÔsƒ?…È{½PËAGN3FGL J1131.1+5810@a¹/ßÁœ@Köõƒ¥À9üÅ0÷ÑÀ<¯k'ö¿Ù xA@@+­,ôU@EP¿`'³¿æÏÇ~f¿èkçÀÕ.¿ÎÅýtNJU¿çÎ^G^
AGNbll@–wPowerLaw1RXS J113117.8+580911?ïÿ}j>Æ?˜œÒ	"?RÏР?˜œÒ	"?ïá™ÍWG?€bM*ìÄå?nôfPåH`?€bM*ìÄå?ïí"b?`y2˜Æò?bøÿ¥¦?`y2˜Æò?ï÷,f‡ÀÌ?=¥"%O?Q§2¦FÙ_?=¥"%O?ïÿ^ù?Ú¹'ˆI?Þ|¢ÙEß?Ú¹'ˆI?ïR¦j"Ё?£ ÇìUbº?•«2¶E'Ñ?£ ÇìUbº?ïÖ:"¡?wÁڂy`Ï?tâñ–vŸ¨?wÁڂy`Ï?r¯Rœ?'ã¥iü?‰ãaéÈê?'ã¥iüAGN3FGL J1131.4+3819@eÄ_Js@Qv‹`òËÀ9Õô†O9úÀ;?)
»E?âð—	qmÖ@'þ'…@"@ "€¿è¦qYg-¿ê¬Ü-Ë¿á¢Ú- ¿ïÿÞ\
¿SAGNfsrq@‰Sݗö+PowerLawB2 1128+38?ïýa܂¼!?2
+–PRŸ?4ñ¤æ?2
+–PRŸ?ï»*¥'m£?‡i;±E­•?5V›¡Q?‡i;±E­•?ïf]¤mT?ƒ–Ðê?"4Ki¾h9?ƒ–Ðê?î–aô;ђ?†CîúñŽ¨?¦™à¿²'Ö?†CîúñŽ¨?ïüºÁY?@tô¡¨ü8?:)ôHŠ`?@tô¡¨ü8?íF-=û¹?¾ÍÚQïü?µÎ–Ø\Ž?¾ÍÚQïü?îސ£ÉÔ?—ëqíG?¢õÆÞN¿?—ëqíG?åð6kÌ×µ?º0'Ì3!?Ô"(fP—?º0'Ì3!AGN3FGL J1131.9-0503@pÒ: WŽ\@JC* dúVÀ9‡;±†ö)À;ž ùt̿햼CxÕ@'
L46@D)ÀmÃÓ¿æ
E")Š_¿ë/gzý;¿ë
r.¤?¶.w•@wAGNbcu@~°ÎX%[PowerLawPKS 1128-047?ïýÛÑ*26?3Ð)'×£?1!vcª¾?3Ð)'×£?ïÚ÷íYV«?…Îü?¼?r"	brò?…Îü?¼?ï©åòì#Þ?-6üïg?…†ƒV%{?-6üïg?ïÿÐìR_Z>ð†cƒçˆj>÷‰éÇĵÆ>ð†cƒçˆj?ïù6N_xO?SfÛ·7mŒ?K&ÅÚþ1?SfÛ·7mŒ?ïAñïhzŠ?§
)ß!Ž?—Á³?§
)ß!Ž?ïMˆ¸º‹?•ÒA$\w?6NàQ¨®?•ÒA$\w?ïùåÀþQC?JϚê»ZX?Hhû°{?JϚê»ZXAGN3FGL J1132.7+0034@pƒõ_þmY@L´Ò_³Ä¾À8x
è³³À;9]¯Þ}?ãÛÏbíû@Æô÷ŽAw@™ _Æå¿Ýߨ¢J˜¿ã	¨ß'¿áÛ£'¬§¿ÝF‹(	AGNbll@'mÀPowerLawPKS B1130+008?ïýšön]?-r%\·-?3(Mžeӑ?-r%\·-?ïÅÄ-I—×?‰½­gZ@ä?}éU´´r?‰½­gZ@ä?ïè&öA˜Ú?l
áÏûÞ?gÙ	³heÛ?l
áÏûÞ?ïw/¹?rÇ/ý½;P?'HÌ]Í?rÇ/ý½;P?ïûp<Ñö?G­E72—e?B=Ã(ÁÄ~?G­E72—e?îcÔI݈v?°s*øò²Ÿ?©Â»frû ?°s*øò²Ÿ?9Þþ?‹1}$[^?‰Ü1\8l?‹1}$[^?ë[h>>?­†ñilÞ®?"¾_Â?­†ñilÞ®AGN3FGL J1132.8+1015@opÛ ¸l@P=@GDÀ:gÍÀ;È©lut ¿÷EJ!ŒAÂ@
¶ža@ÃÉàhÚ¿èh ¼IX¿é…®w™‹ú¿éˆíñ¤ac¿ÃàJK0]žAGNfsrq@|%1ñPowerLaw4C +10.33?ïÿšÒ©°"?§&)•Š?	KM4?¡T?§&)•Š?ïàT8¼_?"3F… Àa?o«Ç†ùA=?"3F… Àa?ïÛÿr?p®ä‡H?rpмe?p®ä‡H?ïÿúY"8>¼O—qs>Ɯ\|"Áª>¼O—qs?ïÿŸærÌ?Ê	ƒ]Q?;5Mâ	•?Ê	ƒ]Q?ïwlœ
?—õ$gò?''gWDc?—õ$gò?ï£àÂŒæ?…À-­h?‡π{þc?…À-­h?ïÿ\•ñÞ?ÁÜ9áUŒ?mG5}Ï?ÁÜ9áUŒAGN3FGL J1135.2-6054@r\åà.©a?ã@?éØÀ7ÅÒtwÀ:°½L&I@‰uҕ
Ä@²,ðÎߢ@ÆÄuw¿ÝxdVRg¿ããõå8Ã/¿åêybru¿ï
$p:PSRPSR@‹eÉþ†ƒ<PLExpCutoffLAT PSR J1135-6055?<Ó°j©£?@!
njÛ
?ïüe‰Ð+…?@!
njÛ
?¡Áp\»@(?¾ÏÊê/ÅQ?îãèúÏ?¾ÏÊê/ÅQ?½D{ÚìË?«r	ä?ì^7p"¢g?«r	ä?,oNáGU?s™ý¸—&ž?ï‹NB¶¼s?s™ý¸—&ž?2ç];›?0`Ã[eç*?ïý£R¦k?0`Ã[eç*?~‹"ƒ
EÎ?¡&pF¬:?ïÂèÖÔÉ­?¡&pF¬:?–'^˜®ær?'YÚt¨?ïKuM}?'YÚt¨?[9üÿ?NÜ>ÿ—ƒ?ïòcvê9'?NÜ>ÿ—ƒPSR3FGL J1136.1-7411@rœn «†À(+Ö@éÕÀ97oJ:¶µÀ;vReþaš?é"ú|C®'@
{JÍǟ@Þø 7­ì¿äÊ<'zÿäi˜¦ï1j¿çNµýƝ¿ïÿ¦CK.RAGNbcu@ƒëIºPowerLawPKS 1133-739?êÎ*û´I?ÄFo¦/P?ÄÇUÈ.Ú?ÄFo¦/P?àµßDŽ?Ì!'N‹B-?ޔAwæãÇ?Ì!'N‹B-?꫸×Ê`?¬Šx5éu?ÅQ£àր?¬Šx5éu?ã«<ÝèX?©¨B¾fc©?Ø©†D/ãP?©¨B¾fc©?àN…xò§t?Ñ>Ÿ´!‹?ßbõ±?Ñ>Ÿ´!‹?´ XVp?¿!jL¾¹S?íkôÿ,+¾?¿!jL¾¹S?âbÑâ>Ê?¹Q«a×?Û:\;ƒþl?¹Q«a×?¶g³E–?™h¹U`T‹?í3	–1
?™h¹U`T‹MIXED3FGL J1136.1+7523@`#W`9%»@Diœ@=òÀ:Žã]2À<*rÉK8¿Ô}聴 @ßF&ñ}@h³ UöW¿ì5=Œ«¿Ü£CÑ9Þ¿µ¥úw™®¿ïÿeiûØPSRPSR@—ªr° ĜPowerLawPSR J1137+7528?ïol}Æn?¡k¿P>Z?'ÒpG2;?¡k¿P>Z?ïç§Ç.Ó'?{´Z›ª?hX8Îm(Õ?{´Z›ª?í[›àNgu?¢R¬©¤{5?µ# ü°Ý[?¢R¬©¤{5?ïíò¯½û×?KžÿÛÕ?b
P)ñ?KžÿÛÕ?ïŠfÃ$ú®?ÆÊúñ•‡?fO,r€¤?ÆÊúñ•‡?ïrçÙ÷
l?¨ijDN<?'£¸‡¬˜?¨ijDN<?í"0Îvgˆ?¤´"™E#?³^yŒº·A?¤´"™E#?ï½:wínÐ?v=ä؀`î?€±bÃÓì?v=ä؀`îAGN3FGL J1136.4+3405@g‹y¢ƒ@R`×óÀ9ß]ÂSÀ;åðL-Õü¿òƒÐ&žzT@½e{C@ ¢àRG¿çƒvãÈM¿ìWDû»*l¿ßýx=uα¿çQB,Ë:&AGNfsrq@x˒:*PowerLawMG2 J113627+3408?ïÿÑÿ3Ü>ñg'‡Æ>÷G×EË>ñg'‡Æ?ïæ-…ìŠû?~kÔõÈ<?iÒyàšÍµ?~kÔõÈ<?ïî…!pÎ?mseôïµ?azÞM천?mseôïµ?ïÿŠx$»?
Vs$?
aòZ¡'
?
Vs$?ïÿãåî>ê*6×ó›>ìܦt7í>ê*6×ó›?ïw´ÖG0&?¢
pŠÊ?'	e<Ae*?¢
pŠÊ?ïèÕîk?t°()$s ?g*û ³+ù?t°()$s ?ï÷ÁòB?M±S:ô\?P|G™Èš?M±S:ô\AGN3FGL J1136.6+7009@`|ŸŒ¨@Fӂ PˆÀ8Û°hjÀ;^R_Hdô¿íxGøI)@²ĆW?ý-;·¿ÓFãh3‰ß¿ßºˆÔ©¿Ü";
dS¿Í¥+OO7AGNbll@¢v¹õY´PowerLawMkn 180?ïùÓ
Ðð?D6ö–âO?K´´,=º™?D6ö–âO?ïßçöì'}?…3h¯ŽDô?pxId?…3h¯ŽDô?ﱀT'î?¤Ë±ƒÃ?ƒŸêÔ
J¤?¤Ë±ƒÃ?ïþè&U»Z?m"D?¢ë?!}–eù‡?m"D?¢ë?ïé–N-?`Ü¢£¡t?fi±ë¼#w?`Ü¢£¡t?ïAg'½4Ý?¦·Jp÷ô?—Ó
Ê2b?¦·Jp÷ô? 3¯¸?Œ,Y×
3"?Š—7öƒ­ß?Œ,Y×
3"?ïêª!•ë©?f»uõ˜"—?eUÞVև&?f»uõ˜"—AGN3FGL J1136.6+6736@`®.oKè@GûrÀü¨À9À®9À;"Í.œ?Òוù&@gғ`DŽ?ûe?õ¹U¿ço@Aä{ë¿Öà0^l¿Ó—öÞx5¿ØF€i"AGNbll@°!ffffPowerLawRX J1136.5+6737?ïþ•L¶oœ?"J–@dšB?&«1 ž{7?"J–@dšB?ï߀ÇÄ-?€Ø}(x?pq¿"ŽÅ'?€Ø}(x?ïÝfˆÜC?w²áösôø?qpL©úu?w²áösôø?ïåLL¬"€?P3¦äWO?j³³O½ø]?P3¦äWO?ïûó¡?B›ÁÅ~³€?C¡¿¼ó­¹?B›ÁÅ~³€?îÑ:ßhʉ?±‹€3¦|?¢ìRs?±‹€3¦|?ïψõ1›?~Kà5d~?xz;ˆ&â?~Kà5d~?ï7Pb)Q?‰ªàP
¥?™ó·f@ù?‰ªàP
¥AGN3FGL J1136.6-6826@r'?…Q
À=™àvpÀ9"Í]"ÍÀ;$É3»o¿ÑW R°Ñï@0˜ZT_S@¯nàˆkt¿çRšNÛ±¿ë>5oÎo¿â™þƒÔ
"¿ç4!ßñBAGNbcu@öͽøôsPowerLawPKS 1133-681?ïø]øaX¾?KˆÓ™´¸?Nˆ''Dn?KˆÓ™´¸?ï•bÈ]c?"4j"œ÷?Š¸ç@*7m?"4j"œ÷?ï'ÇôœÜ?†-Û=O'?‹Ž>i-?†-Û=O'?ïäý‡Cšx?U¸=É¿?kxþ^O?U¸=É¿?ïߪ®{O?q¨;ÆÎ]?p*¨¯êôj?q¨;ÆÎ]?ìuèÜ;Äk?ÁO½3
Û?¼P¹!ܧ?ÁO½3
Û?<´Íc?…38-ò?§ü7FÞÏ?…38-ò?îƒbv¨ä÷?•³	Å5/¶?§ÉؖM—Š?•³	Å5/¶AGN3FGL J1136.9+2551@j¡Ì Õbž@RS&@©À:e¾BÆN.À;¿þraFl?âeë^¤j@}þraF?úÝ[ d¹é¿ëœn<7''?Â_âfšœW¿ëD"†âÝ°?á|«¨‡@AGNbll@½–LÌÌÌÍPowerLawRX J1136.8+2551?ïûa"ÔïÂ?L{ºe¤]}?By°á"€¢?L{ºe¤]}?ïßâP—?"ÎD8l—©?p×Ê.õO?"ÎD8l—©?ïsÉÓÄ?ˆ¶±¯p…?'†Ý``~?ˆ¶±¯p…?ïùK·Ó/V?D£" ""?JÑ ä½™?D£" ""?ïÀØn&àP?€VÇ{™œ?"É\Ë÷?€VÇ{™œ?ïHV²-?¥¼¸Ð¾	k?–ü|¶áˆY?¥¼¸Ð¾	k?îWäPg? AÓç¡£ú?ª·
#âŒ? AÓç¡£ú?ï\¢4j7N?›Ù$ÙZ"+?"k¹wà€A?›Ù$ÙZ"+AGN3FGL J1138.2+4905@bÙ`Ëò²@OðÓ?­"ùÀ:U:ûÀ<Êý¿³àÀYI&‹Ï@1#õ'´Ð@Í̀{æU¿êÿè¿âxnùÝÒ¿ëèé¸ëÄ_¿ïþÒ
ØkAGNbcu@x|9#¢œxPowerLawGB6 J1138+4858?ïү՛'Ž?‰‡ä:¶ç?v¨I¤Ä?‰‡ä:¶ç?ïîc0ðt?híôVRîÍ?aœìԎëö?híôVRîÍ?îÞCc›Ê?ý 4z?¢Éċ‰?ý 4z?ïÿÿñ%ô>h
/[Ž>\d÷Ýé>h
/[Ž?ï¦ã"A°?‰èÄE<µ?†G:7o"?‰èÄE<µ?R¦k? ö AÏ7?Œ—8yÕ)? ö AÏ7?íè"é<«=? ë'k:ò«?°»`¶ö? ë'k:ò«?ïÿø¾m8">Ü@2õ->Í?9ëþ>Ü@2õ-AGN3FGL J1140.4+1529@nM߆ã´@QtUàeuÀ:¤ü4µêÀ;£ÀÌäJÀ
/0ÁƒÃ@	&z?É?ô $ sRˆ¿ïÿè¤Þ`?ï䉗mðH?ÓùÊÁÚ«]?™õ÷­9ù:AGNbll@ÕÉìýó¶FPowerLawNVSS J114023+152808?ïû?]Qـ?SGW+,Íí?C‹[Êú?SGW+,Íí?ïã5²ü?mÁ£Æ.?lÊMÇV;Ü?mÁ£Æ.?î¸GO}tS?ž¨5qY' ?¤{‹	¡Õ?ž¨5qY' ?ïÿÿów>c¶YB_È>YñRÀ½õ>c¶YB_È?ïüº\¡…e?AAú…q‹_?:-Švér?AAú…q‹_?ï|BÿŒ›7?¡QÁí	?w a)?¡QÁí	?ï™=!YÓ?‹"³4Æô?‰°··IªY?‹"³4Æô?ïÿþú‹:Ë>°'¶ÇY8§> Z!·žK>°'¶ÇY8§AGN3FGL J1141.2+6805@`'na«@GÙw·À:%¾<çÀ;ò… ¾Q	?ç`jŠ¶Û@°:6?ùÇ:aOÑ$¿ï÷«z9#…?ïþ9tüèZ¿Å2×BÇ{¿Ëå¢oÔîAGNbcu@»z™ÞÒPowerLaw1RXS J114118.3+680433?ïÿþVÌ?ǽð‹#b?‡¡ŸC?ǽð‹#b?ïØ	h"m?ƒåj«'×?sûKèš3w?ƒåj«'×?ïÞFˆê8²?l ä"q?pÜ»{Å^÷?l ä"q?ロôÎ?h˜c×Êe—?€YÁùªf?h˜c×Êe—?ïýh3x°ô?0|ñ'€?4¾fU;.?0|ñ'€?î½ëpÚfF?±‡‰èÛÿ?¤!Hð¡Í¢?±‡‰èÛÿ?ïÏÂ$ö?xfZÁY^'?x{žýÍ#?xfZÁY^'?ï5£êš,?'ë¯-XŠ?ŸÙK=…?'ë¯-XŠAGN3FGL J1141.6-1406@qg¡Ո]@Fµ| À9ô¤	_$SÀ;¿WÜ_çÇ¿àǬø@&Fæ™R@gãà¢J¿äþøÖ7|¿ç†?
 Á¿Ö¢uµ'®_¿âêM{³Õ…AGNbcu@›"¶®}VPowerLaw1RXS J114142.2-140757?ïÿNõ[ŒC?…qOªß1?!WŸ»?…qOªß1?ïÝ{yÚÓ?€ŽnåˆQë?qBC±F¤?€ŽnåˆQë?ïîŒæý?Y
ÁîO9?asÿ:ƒ?Y
ÁîO9?ïú´¼Dñ?1ÓG϶ž=?E-×½	I?1ÓG϶ž=?ïÿ"þeSÊ?µ&â? 9yE ?µ&â?ï
k«þ)?¯§Ì­Û)Ž?^Ré4ô?¯§Ì­Û)Ž?ïðï&œ†?b -,íùŠ?^!²PÎeZ?b -,íùŠ?ï·°ÛÕ~L?wpk'•—?'ÉØÚø?wpk'•—AGN3FGL J1142.0+1546@n'¨`ܹª@Q"ßÔŽÀ9ßÞèXÀ;´¥hõX¿ÿx9ܾ@2Qç3Ö@^È •¡½¿ß}3£VÂì¿ä€Óð,£L¿äãތ<å¿Ú1מ7
2AGNbll@Ž&Ÿ@¢‡PowerLawMG1 J114208+1547?ïþZjüðx?&\òøà‰?*YS틳Ñ?&\òøà‰?ïâòx$vN?'o=…ˆž×?m
‡éH!?'o=…ˆž×?ïÕÀIdUž?s
Ü<ú?uÛYƒÝ ?s
Ü<ú?ïÿù
 
>Ç-2—|H>Ë؇»@YP>Ç-2—|H?ïüßޑ44?=ø-?ª˜ ?9
g㆗?=ø-?ª˜ ?ð/]?šÃ&­T;µ?ŽCéë"Ú?šÃ&­T;µ?ïOð¿©µ?'¬ëëQñZ?–ÿí23^?'¬ëëQñZ?ïþü\(í,?%"GU¯K3? :?À¶Ñ?%"GU¯K3AGN3FGL J1142.9+0120@p¹7ß (@M·ç 5)­À9Ì·áƒ=7À;Õ§uû.à?ö!sЇA}@
«¼±Ì–?÷Y©™èt¿Ù™‹Ð5ë}¿ÎðCgó7¿ÜN×+܎¿êÎd~§[PSRPSR@œšwškP±PLExpCutoffPSR J1142+0119?í"fÝ=?»öÊ´Ï"?³ÜÉãñþ÷?»öÊ´Ï"?íû՛Iê?·U :–?³x!To‹,?·U :–?é˜B2ØÌ?°£ž^³O?ɞ÷7ÀœÏ?°£ž^³O?é­íòiòë?¢n"ƒb?ÉHH6X4R?¢n"ƒb?æâ7òšg?ÇäšÐ6Ÿà?Ò;'ÌË2?ÇäšÐ6Ÿà?åÛL«Äh?Ëրln_¦?ÔIf¨wû1?Ëրln_¦?ßL?É!?¹Õ¥ÿҊ?àYñàwï?¹Õ¥ÿҊ?ÚÃÁѾq?´1öÆf?âžyŸ È?´1öÆfMIXED3FGL J1143.0+6123@a® ý;*@Jïä ()À9`¸K5ˆxÀ;ºÜ8zšÑ?ìX€ŒNϾ@}ö۔í@+¯ >ŽÜ¿àFc'²°Ó¿Þ¨ÑM˜˜¿Þ	©æ²•Ù¿ç?+õsAGNbll@™óóœ¾àPowerLaw87GB 114026.7+613850?ïç_Dß/?e'0%™o?h »^éŠ?e'0%™o?îI8s—"õ?§òݽëU?«lxƇ°°?§òݽëU?ïœá6*"W?¡ÈÞm?ˆÇ²k(–B?¡ÈÞm?êĽPÐI{?¤²
'?Äí
¼¾Ú?¤²
'?ïS-uÈÈË?""fŽOD©?•šQE/£?""fŽOD©?å·Ü`ú¨?̟ܲP¨B?ÕüG>
°?̟ܲP¨B?îb̏ €?¤øñÞFJ?¯ÉÓ:}"ú?¤øñÞFJ?Ö[mÏfZ'?²ùä³Îm?äÒILÒì?²ùä³ÎmMIXED3FGL J1145.1+1935@myA HàD@RBî?äžÀ:Š"#8mÀ;õÙ&wc?®ÒDHî×@
ĎH­˜Õ?ÿ¡7€ô7¿í+ÈÐé¼ó?Äé3ÍY\	¿è±Ëi W¤¿ƒõ­…x"AGNrdg@ªv£þ\'ÑPowerLaw3C 264?ïü@²U[?B%æ]j??]û(î»?B%æ]j?ï῕#4°?'	üfA?n@j R0}?'	üfA?ï²M…¢tg?tÂ9«V2?ƒlžœŠP+?tÂ9«V2?ïöE†i]‰?C7ùQ"?StòÍÞ\?C7ùQ"?ïæ'súp?m‡³€ß@?i}ûbÊ@$?m‡³€ß@?ï7åኍÒ?®=l­^d¾?™CË>©Ê?®=l­^d¾?ï/Whih?'ýcñ֗]?šòÝü?'ýcñ֗]?ï:ЦK-Ñ?–)x{:(³?˜¥ë:	áâ?–)x{:(³AGN3FGL J1145.8+4425@c}ËßÒc@Q[ÖÀÀ:ß­FÈBÀ<B‹•ÊØ¿§j9DZ`ß@"óM¿üZ?ýšRaKÊY?愈bBH¿Õc8ÉöÑ¿ä:kc{O'¿Ê…û¨¾‹ÓAGNfsrq@¬+´`ªdÃPowerLawB3 1143+446A?ïü%Í;~ÿ?I°Fä?>ѕ9ÕàO?I°Fä?ïà¯öŠÐ?ƒ32"J?oPæì˜x?ƒ32"J?§ˆ?‡F%R?Œ?šYf?‡F%R?ïíïév?'?Qs;=`?brc÷?Qs;=`?ïö
7³ÂÝ?Wê!åì;?S됅<v?Wê!åì;?ï..™­?¨˜a¢f¯¨?š:,Üün?¨˜a¢f¯¨?ï@8‰îÆ?"G_€?—øýKR‹T?"G_€?îã]Ô?žÄñ4€Ó4?¡Îº2¢[ã?žÄñ4€Ó4AGN3FGL J1146.8+3958@dŸÙÀe¶=@QÝ­À,«ZÀ7ê$gMÀ;[(fP–ñ?î'l ö«Õ@óN¸IÝð@çÀC&›¿âdTÆßV¿å14œPz¿å^›ÎÔ¿ç蔘AÅAGNfsrq@í2a|ÚPowerLawS4 1144+40?ïÿUñ¬³°?Ū¡`š?ÂÀ?Ū¡`š?ïåО$?'ˁX
<é?jèî†dd?'ˁX
<é?å^ØÂ?‹SQº•?ŒÓF¤Ú3u?‹SQº•?ïþÖ?šÓ3?S*µÛ·?"œß*C(?S*µÛ·?ïþáu·xc?#øÒæ†2?!è Ë敚?#øÒæ†2?ï€U¶sw¥?–;Lµ¤âÚ?ê'\BÞè?–;Lµ¤âÚ?ï`´3-?ã'Ÿ@ÈS?"é~½bp?ã'Ÿ@ÈS?ïýŠZó|Ë?2ǿƀ•?3­(;ák?2ǿƀ•AGN3FGL J1147.0-3811@rß 'á@6ø;‡}À8¦ìAÝ"À;l©èœ6,?ê4G;9"G@no+¢@îàrñå¿á¨g€þÔB¿ä¦÷»oÉ¿â®
Á"Žd¿æBDý¤Ê¿AGNfsrq@‰¶"£Y6PowerLawPKS 1144-379?ïþþ9Ñ¢?ÁlL/f? mªo?ÁlL/f?ïËïSy=?…ƒt"Ãw¯?zV3'ýg?…ƒt"Ãw¯?ïÇï‰K~ë?'!êÈì?|;kn–"?'!êÈì?ﯛÕoCì?bU/M<|?"
©Vo?bU/M<|?ïþ<ç¬?1(¦Õ—:?.n¸2ù‰ê?1(¦Õ—:?î"æÞé&l?´®$ó­ËÑ?¦±'I€=?´®$ó­ËÑ?ïqð½í¶Ò?Sœuœ-U?'Áè>ى¾?Sœuœ-U?îK¤ï'?"*Ÿqçý>?«Oµ´}+Â?"*Ÿqçý>AGN3FGL J1147.8-0725@qJJ '§@JÇÀ'áÀ8ÊoÖQ°ÍÀ;g9
É<?Üú(t,;Œ@íËA\k¼@‰V  žñ¿ÛÏ|i¿åå»ëpk¿ä®<ì%¿ä(ï¸_,‹AGNfsrq@Ž‡²ßP]PowerLawPKS 1145-071?ïÿp½F5Þ?Vu(Ä?èUÄÀ'ß?Vu(Ä?ï֕ÿ¿œ?‡cÞV?tµv—}‰ê?‡cÞV?ïÝÙï?ldÃh:ø?qv>FG?ldÃh:ø?ïùìñì}(?-žÂÈ+Ù?HL7yÖ¶I?-žÂÈ+Ù?ïþæ锿Ñ?#k'"Í­,?!'j\˙O?#k'"Í­,?OcY?²'"ùÁŠ?.ŽÞªšÉ?²'"ùÁŠ?ï'ýÁ-Õ?Š´-Q?|@"$&Ô?Š´-Q?ïÞË-_à?c¥à?pšyÖ@S?c¥àAGN3FGL J1149.5+2443@khÌ Õbž@Rø. &{•À:SYäwä=À;êúµ=d¿ù"øzût@RK»jNÓ@ã"@>^Š¿éI \ŽBÆ¿ÔmPëªÞe¿ç%+~ðI¿à±60"›©AGNbll@©¦jÀƒoPowerLawRX J1149.5+2439?ïþ.‰vƒ?(ËäB74?-©¢#ÖO?(ËäB74?ïä֏ øQ?ƒ¼@ùr"Æ?k)pËÉß^?ƒ¼@ùr"Æ?ï¾W¡¹?su¹lª¤?€zjFF=®?su¹lª¤?ïÿâĆ>æBL}Ï>íéúXo6>æBL}Ï?ïúÐä'ú?AŸ]ÆÆ­?D¼n¸ˆÈ?AŸ]ÆÆ­?ï‰"'O¿Ë?"À¨q汬?·_rïEO?"À¨q汬?ï^ôV íî?Žý®²~™˜?"!u1	¬4?Žý®²~™˜?ïû}b4I?H€ýI¹?B
wõÔ[Î?H€ýI¹AGN3FGL J1150.3+2417@k¥Ë èBt@Rþ)¿ìêzÀ8ÛðòFÀ;Q†Xt5\?½×ë4¨Ž@"úõT*z@³&ÿô"¿áظÀrù¿ã•Lo:P¿ÞyLOÂh£¿è•ñÐ"¨ÞAGNbll@—L&Á½¥PowerLawOM 280?ïò?"«?j†)X ù?[àáhýzÙ?j†)X ù?ïߪ"£µ?'é?³Äõ?p*¶KN݇?'é?³Äõ?ïµh-?‡vŽÒ–:j?'»åó1"?‡vŽÒ–:j?ï¿èrÎ?eséÏA'6?€>Åߏ?eséÏA'6?ïæÏ8H,%?pc"G?i0Ç߯Rë?pc"G?ï `Ë=?§YYéy''?óþfc?§YYéy''?î·9©*Aƒ?¢dW«S#•?¤ŒeiìKÑ?¢dW«S#•?íRâ¡Ìª?¥*S¯Hi?µhïû́®?¥*S¯HiAGN3FGL J1150.5+4155@cã{¼¾b@QªÍßòCÀ8P,‰ËÆ=À:î"Z•wÌ?èÚÈ¿™U@Ü"¡À…?ü$PôF¹¿Ñ¦àvo?u¿Û©S1¿Ù
ª©ój,¿Ê=.‰«:AGNbll@£±­à
qPowerLawRBS 1040?ïóÈ8,[?TjGÖà[?XoîÁ²q?TjGÖà[?ïÔ_yüßÿ?x,= ŸrL?uÐB÷A,«?x,= ŸrL?ï'P¾o£?‡1Å'›?‹«Ðg†Øê?‡1Å'›?ï/aAŽj¼?é¼´¶1?š×ÊÃy?é¼´¶1?ï¹Mç>"?Ôž¼"L?¬†1('?Ôž¼"L?î#"Ð×ÉU?¶ PLɇH?­ÆÂô;8¬?¶ PLɇH?ïW³Nw˜?'oó‰'›?•	—èÚî?'oó‰'›?êš(]ŸËë?´âuƒ^ä?ŗ^‰€ÐS?´âuƒ^äAGN3FGL J1151.4-1346@q—¢ŸœèÙ@GIZ _†xÀ:(8_ÂÞ7À;¿?']<¿Õ-Âvî°@éi{Ð?ÿ«@àoí¿ÜZ§žó~¿çÁ Hõ½1¿‰s¯,Ü`¿Ýpà~‡½AGNbll@©Šš¹õY´PowerLawPMN J1151-1347?ïÿ/j{Ê?'ª~â¿?´/:ÿ?'ª~â¿?ïÞVÿ@=?€˜0"¾´Á?põTˆžñ²?€˜0"¾´Á?ïìG}'?X¨b_õ¡Á?c¸÷n;:÷?X¨b_õ¡Á?ïýµ'¶?IJn?2Ssv¿q?IJn?ïÿFÆ|À_? } ã?'/Ãèa? } ã?¬U?±Æ?´Ä?Ÿì

u`?±Æ?´Ä?ïæuÐfµA?pcµy•^?iŠ/–‹E?pcµy•^?ïò<7é¦L?S?-Á?[‡5Gb?S?-ÁAGN3FGL J1151.4+5858@a(¿;ê'@L>­¿ÁKÀ9iëBÙÏÀ;¥ÒÐçÝ.»™›@PÍåüs®?þ­&žû-]¿æÑØú†€¿ÙíuÝ/y¿àÖ¾ù$™'¿ÊŽ!%–ŠAGNbll@£Ò Þ҈ÎPowerLawTXS 1148+592?ïþa'Î? þ'ÛÙɬ?)ç
ç¥Ø? þ'ÛÙɬ?ïæyaž^-?×œ¬š
?i†žƒýêÁ?×œ¬š
?ïã­!òÕ0?hê™Y_o5?lRÝßÏ÷å?hê™Y_o5?ïÿnjõI÷?jø·Pñ?2©´š\Ý?jø·Pñ?ïüà"ÿG?1¾OF(º—?8ûÖú•+?1¾OF(º—?ïd&ó|?¥é´zu°ê?"|»:É'?¥é´zu°ê?ï¹´ÍQ­?ƒùí\†^?ºR´¶Ò?ƒùí\†^?ï÷ Ç1®?P¢¬soŒ?Q¾qH¤Tû?P¢¬soŒAGN3FGL J1152.3-0841@qq_¿ƒ8.@I¶hÌÀ9(ÇôøÀ;"°Švæç¿ÝÆ Ò@""†g¹@Ž=Àâc¿æO&ŠÈ	]¿ær^E"_¿æç$˜`¿ßf¨ÎôL÷AGNfsrq@‡½ÈK]ÌdPowerLawPKS B1149-084?ïÿ³)–/
?I¤Ʌ%?5™;ŠZ?I¤Ʌ%?ïÝP¹½Ë?LÓ©G?qW£'¬?LÓ©G?ïå5&õ°?e(¿§J?jbÊËKà'?e(¿§J?ïþÿ?'µšÆ-?/À! ns?'µšÆ-?ïÿr*X²ã?\9NàÇ?º¸"MpÄ?\9NàÇ?ïL×é$` ?¤U͟­Z?–eÝ+Éð?¤U͟­Z?ïÊÐÃHáé?}öí¯à˺?z—ž?b?â?}öí¯à˺?ïáèïÔ?eBYA÷?nðbïc¬?eBYA÷AGN3FGL J1153.4+4932@b0öÿ:Þ"@P=ÿ%¿­À8Aó‡K¹<À;–w§×Iþ?éCVqÚ@†@I~úï@A{P¿ãÅxãŸ)Ú¿å"ZíƒÈï¿ãIŸá‡D¿ìÁA_yAGNFSRQ@€^=<64PowerLawOM 484?ïû'"ٞÂ?=
(ã…ù?CcuCñ•Þ?=
(ã…ù?ïç0Ù;Åÿ?{Š}Eª?hÏ&¨½!T?{Š}Eª?ïm¬¸-×?‰žrßU†?'Jhõ[
!?‰žrßU†?ïÿë¶Oj>Ö¶¾'Œˆq>äIÅF¹>Ö¶¾'Œˆq?ïú˜pxY?H´×ˆ¹ý?Ež@`_Él?H´×ˆ¹ý?ïƒHE­Íó?•E²'4@\?-îžÛW<?•E²'4@\?ïLÒÉ'¾?''\x Ú?–e¦ÛžJ?''\x Ú?ïÿ厘<U>ðÖXG)v)>êq"/ËÕÆ>ðÖXG)v)AGN3FGL J1153.4+4033@d`Ï‰@Rڀ¶–À:wŽF@À;ÙUËäo?ÍòÒ_*w@Ú[Ü®l?üF!_K??ïúGþÿ¿Ò'¯·µ…Ö¿ÒÑ;Ïíq;¿ÚÝx-Z£‡AGNfsrq@²Ê1&éyPowerLawB3 1151+408?ï/(°‰†b?º±»¾ {?šéíeº?º±»¾ {?ïÜ\Ø{µ6?…ó‡÷…³?qѓÜBm?…ó‡÷…³?ï¤mYìý¼?ˆ,mœH‡?†ä©•îœß?ˆ,mœH‡?ï¿ËdiÈ?gã°y:­?€
&ô~t'?gã°y:­?ïônät?s}"8׏?W#þOºG ?s}"8׏?ïÄõ+Õ`?¥µeÏ6?gacYþ?¥µeÏ6?{´4?"™2¦Û?˜ab›j?"™2¦Û?î7ËgSÓ? 	ÁQ9F?¬ƒI''Æ? 	ÁQ9FAGN3FGL J1153.7-2555@qðe¶™…@A"Œ_õ3À: öC¾›²À;à ɤ#`¿ÊF#.§@
ˆùyO!@9 4¾N?ìÕa¤h]¿è"ÍñÔ²ä¿Á7æÁj˜û¿ê8חAGNbcu@¦†N}VlôPowerLawPMN J1153-2553?ïôÛؔ'Z?V Åm>1?VHN'#~?V Åm>1?ïÖÆ8/$?'Y\?ÙxD?tœä$þ?'Y\?ÙxD?î"<Zj|?š¤¡w˜ï¤?¦¼?ì&<?š¤¡w˜ï¤?ïï!t2N?K—ìÛCš]?`Þè[³)ð?K—ìÛCš]?ïî²#œ4?aÞøÿö¼Ö?aMó*üŽ?aÞøÿö¼Ö?ï!V®ÚÀÎ?ªi3nn'?›Õ*('E?ªi3nn'?*Ë'?™ÃìVêmS?¤tIʓ?™ÃìVêmS?ïÌ{™(†?'//«á:?‹Ìá ••?'//«á:AGN3FGL J1154.0-3243@r²gÇ@<œûÿÀ? À91ÃÇkÀ;iEW"&?ï­qpì¸a@I¼ˆ†÷«@lÅßȧú¿Ü‰I±5'æ¿áˆý&~;g¿Ü@Ö²÷¿æ¾üHÕÆAGNbcu@–›#S&PowerLawPKS 1151-324?ï¸
 ì8?c_g›O?ø|Š¶n?c_g›O?ëcŒËï›ó?¸òx¸?ÂqÌÐA2?¸òx¸?ïIõôR;¦?wÝ!ÒºW?–ÁAzßõ=?wÝ!ÒºW?é/k‡2?œ¹]8¨-ª?ËCâS­ã9?œ¹]8¨-ª?îrÂ&‰?ªÅ`ۂµ6?¨ÓÝ =à?ªÅ`ۂµ6?×Ä`ðŽQ?Ì}ÏlAû+?äýO‡¸Ø?Ì}ÏlAû+?ìÿWfCUë?ªf£Û¹e?¸DÎSD'?ªf£Û¹e?҃xJ?ª]ÞܳŽ|?æ¾1CøZù?ª]ÞܳŽ|MIXED3FGL J1154.2-0010@qå¿­)™@M¶xßå®EÀ9ÜW?öÀ;r¤Þq9ÿÀ|v4ÐR@¯9"õjÑ?úð ¦=¿åô"½Ö¿ÝÜSH¿Ô÷"}~c'?£ÀÌó&JAGNbll@¶;o\(õÃPowerLaw1RXS J115404.9-001008?ïÿ9˜Ê^*?^vç¼j?ÌèQ4Á)?^vç¼j?ïÞo –šÙ?ƒ}'p?pÈo¼A·u?ƒ}'p?ïã ø.`¢?x÷NÈrò?lßџ^C?x÷NÈrò?ïÿÿü=íe>@k';ÿ¾>?Ì<Çñ<>@k';ÿ¾?ïþù7cïi?ƒ_¿bc? lŠ2gÕ?ƒ_¿bc?ïiÓz³Fá?¡©(iìÝØ?'Ő¦'‡Þ?¡©(iìÝØ?ïߥVˆš:?{ò¯ØÈË
?p-T°6ë?{ò¯ØÈË
?ïÿÿŒ' >˜
"¨ì:z>ŒÞLÁ	#">˜
"¨ì:zAGN3FGL J1154.3+6023@`é¦Þüz:@K¬ºAn_À9‹æYeÌãÀ;Ã^Zÿ*?â,š-±@{ÅËÑ¥$@AÚ?üð+¿Ö\Ù²ìÆ¿èy˜㳑¿ìšý‹ K~¿å$r3µJ`AGNfsrq@'2ßP]PowerLawRX J1154.0+6022?ïÿ˜Ý9µ?Ò҃œj?	È©é5ÞM?Ò҃œj?ïÚ­$?‰ØIJ	?r©qZ噗?‰ØIJ	?ïiÑFrïÐ?ÎÙ$Ešï?'Å×5¡ì?ÎÙ$Ešï?ïæÆòmE?Oîð•Ïa×?ið9@lòg?Oîð•Ïa×?ïþ"ªÊ'?-VÑïÖÈ3?'µP	>CÖ?-VÑïÖÈ3?ï;pÜ—+?¨³S;&̼?˜'ä"Ô"Š?¨³S;&̼?îÚß\úàd?š–Sz6¹?¢R
,â]Ä?š–Sz6¹?ïKC†x¼?k'm¯?œ–—‹ÁLŽ?k'm¯AGN3FGL J1155.4-3417@rEߨq¤@;(Ràw¤|À:Š…=ÂÀ;š®]uüÜ?ÚÃèNÕÈk@gD¡D³¹?õ]ß>>?ï†	‰ÍI¿ä–.ÙÃfƒ?¯zH<ý¿ÂxrÜ°3~AGNbcu@̇\)PowerLawNVSS J115520-341718?ïùš»'¢‡?Tô+%¶"?I•Œõ¾?Tô+%¶"?ïÉkÞWu?ŒˆôÌ>^??{JüCá@?ŒˆôÌ>^??ïc‰'¹ó?'8@Ã|‡‰?"œÎʁW©?'8@Ã|‡‰?ïí!Ú"ÿ<?Prªè܂ä?bÞ&Ü;µ?Prªè܂ä?ï󤬿ˆŽ?b%J˜€'?X¶¦‹í£û?b%J˜€'?î¶Èˆ?µãTE?¤ž"~w=?µãTE?ïkɬ~E"?'µ—"*Õ?'†Êp7[È?'µ—"*Õ?リ"NÐ?wJ*+?€YÛ9‰P?wJ*+AGN3FGL J1155.9+6136@`Ʀ?šIÃ@K%v¹ÃÀ:Ïÿt¿Å}À;÷û'Ü5ö?áõûÏS@8H‡®4±?úVÿn4¼¿íÕĘ©bB?ïÛ ±•'´?®ÅEÞ M­¿àÐ3xl<AGNbll@¸³¹‡+PowerLawSDSS J115548.40+613553.8?ïþªãCä?°`"¨º?%QÌ­»°U?°`"¨º?ïËðõ(¿?†ÚxuÌN¼?z…_ñÇI?†ÚxuÌN¼?ï»÷¹Ïu?'G¦æëÓ?«5¼½?'G¦æëÓ?ïnû¿î0ä?}ÚE²™÷?' ˆ©n?}ÚE²™÷?ïû\ÅRÚî?>Ê£(¾$?BŒê`wpØ?>Ê£(¾$?î†Ã¼éæõ?°i"Òò?§"Ä0…©¯?°i"Òò?ïgÉU§"ò?'¦{ÖðO#?"ÕLÇ/´?'¦{ÖðO#?íäÿôõéY?¦ øªîx?°ØZƒ3?¦ øªîxAGN3FGL J1156.7-2250@qìò?î,™@C'.ÿÇËÜÀ:='¡}"À;¢£Ìhú?à`ðúP@
/FB¯}?þ=~`X/l?ï¶z'A&¿äQƒ¯½¿ÙumKv»¿Â£¼y© AGNbcu@±Î!-w2PowerLawNVSS J115633-225004?ïý­‹°?5*Ëb	)?2"¥Ûñ[–?5*Ëb	)?ïÑv'­ ¾?…ªG(íæÌ?wDì'é\?…ªG(íæÌ?ïÌNèplO?uñÌä‡B?y؋ʉˆ£?uñÌä‡B?ïقv×·?]¡wáoex?s>Ä­4Ô8?]¡wáoex?ïúщ?CWÄ(•}Ž?D»ßê"Aé?CWÄ(•}Ž?îõ ·+?£"_m§7? ¥þ\ñS?£"_m§7?ï Ù~Xlö?…£Ck®‡?‡É w£2q?…£Ck®‡?ï
Jà_7?'Ø'7¨7í?ž¶£ð©ƒ™?'Ø'7¨7íAGN3FGL J1158.8+0941@p­ÿ'+¿@Q&^è¬À9•,D+¨ûÀ;˜È¡ÄáFÀ0°ÿç¬L@«=ø9à@R"`R%<¿Ûiís¡Ÿ¿âì3ˆ©Ão¿à©wÍA¿Ò;'§%ãAGNbll@Ÿ?y#¢œxPowerLawGB6 J1158+0937?ïÿb™°É??XŽ:¼£"?¬Æ'¡e‰?XŽ:¼£"?ïäuPS?€d%íD#?kŠàǕ%M?€d%íD#?ïï¦ÿ2Ѝ?eEÆþ=n?`YhBÝ?eEÆþ=n?ïÿÿ&Èï>˜˜8‹'åÊ>›=\¿{ý'>˜˜8‹'åÊ?ïÿ,í6?µ}5Äâº?bc®Å_¤?µ}5Äâº?ïpwá°V?£ß7ÕÑ¥œ?'ñÐÔu6?£ß7ÕÑ¥œ?ïÓKÓ¬Ô¤?´%}êCÝ?vZ(åÂ1?´%}êCÝ?ïÿåÌU·>ñü*
L˜d>ê3¡HM.Ê>ñü*
L˜dAGN3FGL J1158.9+0818@p°ñŸŒ¨@PÜäÀ™,À:§ÎçY@À;ð?HkÈ¿¾ç­xɕ`@¶õlÿÜ?ýéeŸA#a¿ê|Aâx…£¿Óûãl˜Ò¿ÅwKu
7¿Ù­/}ñóMAGNbcu@°;,1&éPowerLawRX J1158.8+0819?ïþëi+Mó?A¡ûÇî˜?!Inƒc¹0?A¡ûÇî˜?ïÝuh%Çÿ?"¯qˆˆ™$?qELÉl%?"¯qˆˆ™$?ïâ¦
k=ç?hXÕÈWé?mYõ¿]A/?hXÕÈWé?ï÷Gð.¦²?;l¼/ؘP?QpÖ쬭?;l¼/ؘP?ïýS-àŸ#?5(×*?5f'jâJ?5(×*?ïAÒèðš?¥í–ؔ¼?—ßÅ©Á$»?¥í–ؔ¼?ïÖé˂—A?sJ¹‡)»I?t‹VÁ£f?sJ¹‡)»I?ï¯wÏì.?|žÜþ‹õ6?""2~–?|žÜþ‹õ6AGN3FGL J1159.2-2141@qòs?Èlì@CÊÍ_™Ã‹À8Û¼¸''íÀ;>£
¶¡è?×Ò8ôŠ£T@Cˆ™A/@â矶ê¿âóâhž¼¿æ¡y™ÁT¿æiùB÷vo¿àôÓ;YÏAGNfsrq@'mW$tSPowerLawPMN J1159-2142?ïÿG¹'(Ž?¹&\°î?ÝÃNú?¹&\°î?ïÚ#W>‰?»<ê­Ç?rîxVp?»<ê­Ç?ïÝIh˜‰"?k}×¢
ýÅ?q[K²[^'?k}×¢
ýÅ?ïû}¦bĊ?%Äíu—v?B	gbù,"?%Äíu—v?ïþ,™ør?,ÍHDuôœ?-6dobå?,ÍHDuôœ?ï°rזˆ?±·òNîMò?œiñ«ìfø?±·òNîMò?ï‰å?ˆ<ìÏ´y=?¿{;Æ»Í?ˆ<ìÏ´y=?ïäã_éÓ?^ÕكoÙ?kîm;õ&?^ÕكoÙAGN3FGL J1159.3-2226@qö`RP/@Cma .QÀ8…ž8dË\À;ÍèU¿O?ñ_ß0§'¬@&æÓE7@ùSŸQí¿å\¯:ëŽY¿äZDiÁ¿äªP!Å;x¿êŽã4îVAGNbcu@'	È´9XPowerLawPKS 1156-221?ï袸a?jÐ"Þ‡9?g=]xìþÙ?jÐ"Þ‡9?ïÇË8M#t?'Ïå¤í²6?|cã½Ë?'Ïå¤í²6?îÑq¼}@À?˜{5r¬¤?¢èä8+ô?˜{5r¬¤?ï±­%]§?c6œÊՕ?ƒ"¶ŽzŠ=?c6œÊՕ?ïÛ¼™£Õˆ?y£g³y3?r!³B²ä?y£g³y3?îùû­ú"s?¬°qºfõ? `E!2¯Ê?¬°qºfõ?ìE"×
?ªÈŒY캼?¿ÿ}ÓYG´?ªÈŒY캼?îÈZf±m?'†®Ÿ)e?£~]…#?'†®Ÿ)eAGN3FGL J1159.5+2914@hî?àH@S—úÀ%À75#Â|ç²À:ؽØ=CW?÷¿·e‡n@E|^Jc&@éý¿]ù¿à7Æíî8¿ã"<b3¿äÂBÀ
¿äcåj}wOAGNfsrq@{v	"SLogParabolaTon 599?ïþbs4!'?)8ÜÏZï¸?)ØÉ$'Ö¬?)8ÜÏZï¸?ïëǁçÔÄ?j)ô´"?d8}õÏ$–?j)ô´"?ïkïˤP?G&û¯rÑ?''äÓ§þ?G&û¯rÑ?ïÿ†¡"»>ÿÔӶڀ/?W±‡U!>ÿÔӶڀ/?ïýq}ÏAO?3WU)Zî?4t¥,‰?3WU)Zî?ïc:^Âû_?¦ã*<]W?"˜´$0ø ?¦ã*<]W?ï‡ï®Vȗ?¢åš9'?ŽjMÚ1?¢åš9'?ïÿ‹¼óL$?
ÀÀ4<@?
»o4•³?
ÀÀ4<@AGN3FGL J1200.8+1228@pX: WŽ\@QÊ9`~TÀ:ªŠ'¥aÀ;Ò7yê¿Äf!‹Ú­û@GðÂJgØ@üµ?½Z>¿ãɵî¹Ü…¿Úôê-ðÖ¿èäXòµi¯¿Ò €³2ŒAGNbcu@•Þl1&éPowerLawGB6 J1200+1230?ïú!¦Ô?Ps{h`ã?Gyg2"?Ps{h`ã?ïÞJ7•¶?ƒØªÂ´	¥?pÚäc0Á?ƒØªÂ´	¥?ï¡U±Ò?€nò®‹'?‡»jšj´[?€nò®‹'?ïôeè,?Dç\À×=m?W5ôG&èr?Dç\À×=m?ïÌïÍÐ$?","XxAN?yõØÝØ?","XxAN?ï8üÿÖ œ?ªBꃓ‰9?˜à`'}?ªBꃓ‰9?îvq•¢?¢VlûÚ@#?¨Ÿêz>?¢VlûÚ@#?îãÒÌ&oç?›mœè7õ*?¡ÂÓ@,¶"?›mœè7õ*AGN3FGL J1200.9+2010@n)<ßï¿@@S!ãŸâˆ÷À:»˜¢úÀ;Ô O*à~¿øâZ=8DÀ@;ªv`¯m@1Œ` ÿ"¿æ0o<+ˆ¿ê?äߓ#¿àvºól¯è¿ïÿåÊ/õ¢AGNbcu@…Ç-b8Ú<PowerLawTXS 1158+204?ïþ™r¤¯š?%?`§Ýb?&hÕTD˜á?%?`§Ýb?ïåWe˘?~vÖú	à@?j¨šFÊ`'?~vÖú	à@?ï€I!Ã/{?ÞŠ‰æ.,?í·'£½&?ÞŠ‰æ.,?ïÿšø>jŸ?Ñ$2ó4h?	Aî¹ÚÐÝ?Ñ$2ó4h?ïÿqÿï~?šG#à7W?ÀßCŸ?šG#à7W?ï[~÷ý×?§_´C®ã?"!
.?§_´C®ã?ïŒGYŽoM?ˆ™ùC]?Œî)œd,Ù?ˆ™ùC]?ïõ_©™ýÿ?S<|ç•þ•?U@­ûB7?S<|ç•þ•AGN3FGL J1203.1+6029@`­ñ¾ôœõ@KÑm`U«-À9qɕà§À;Ô#ú±¦¿ø4€z¹¯@²:)Çy§@ªþ¢Lœ¿é<*Fê9¿ÞíÆw'¿á»qä'¿ç™Ä»¹ÞAGNbll@–>ºxl"hPowerLawSBS 1200+608?ïû–Ö4™T??'ã˜Øók?A¤§hmšþ??'ã˜Øók?ïê\—Û~k?v°ïŸÖ6½?e£h4?v°ïŸÖ6½?ïÕf³Wº?ušÿğ˜h?uL¦^¿w&?ušÿğ˜h?ïÿ"¡~¯!?ð}O^‰Ø?כ·È ‰?ð}O^‰Ø?ïô1;ûóp?UàBxàz?W‡ÓßÍ?UàBxàz?ïr1ãÒÍÃ?›$£
æ¼?'¹Ã€~ݯ?›$£
æ¼?ïWßĐ.?"¸´ÿàý?•qov3?"¸´ÿàý?ïñoòbü?`~ïˆßC9?] Õþ·œ?`~ïˆßC9AGN3FGL J1203.2+3847@dààëgÃ@R¥ïß÷KüÀ:k'öjÀ<q/îU¿üÐÚ8M´@fÝ°õ«¾@m!¬ˆŠ¿ãAÿÞЎ¿în-{°?ݯ8gOšr¿ïÿöõ;ŽAGNbll@²þÅm]PowerLawNVSS J120257+385147?ïËÿm'†ƒ?§¸É`æÞ?zIò…?§¸É`æÞ?ïåfq–Š?'³BŽ 8â?j™o‹©Åú?'³BŽ 8â?í{g3¸5³?¤"'<´Ùi?´$Æb>Re?¤"'<´Ùi?ïÿÖĔ¼]>ñŸ^)îϕ>ô¦íi<>ñŸ^)îϕ?ï÷›Íö'?'ôlbü'ó?PÈf?ð¡?'ôlbü'ó?ï`jÓªÙÕ?§×™tÿ³?"ò¥'ƒýN?§×™tÿ³?íqÓY®Çÿ?§v8š¡
?´qe3e§?§v8š¡
?ïþ.F9?8s3¾3ËY?/¿	BrÔj?8s3¾3ËYAGN3FGL J1203.5-3925@rO@ €@6ƒËßgDÀ:2.¸z/qÀ;—øö ƒ-¿½ÄfÑ	6N@
"Z"
kê?ú7Ó@"TŽ?ì;dÐ9=ä?ïš[ÓæF›¿æÐ3¶Xu?¢¥½‹³ŸLAGNbcu@¾²ƒn—PowerLawPMN J1203-3926?ï÷‡ÙRÂ?TQ~[f?PðMÈoKæ?TQ~[f?ïÖFT|?' mì•0©?tÜÖ¾:?' mì•0©?ïTÇCk²??QŒJã?•gÒkÈ??QŒJã?ïùšËjD??BaG½'?Kᔹ
"??BaG½'?ïËê®×eÏ?')À¹D?z
¨'o i?')À¹D?ïÃ#";a?¬1òÆz†?Ç›paê?¬1òÆz†?îªþN'¢?žòqòßÒ?¥P!Yþ?žòqòßÒ?ïž"A•Ãî?b¶Ÿ"?ˆwo¨MtO?b¶Ÿ"AGN3FGL J1203.9-6243@r˜n «†¿ÖªƒÉbÏÀ7Û5÷2ÑäÀ:*Eå"T?ü$NÂÜ@Sjøœ^p@.jÑ¿á'YŸX…¿åÇVVVu¿çP§'«"¿î'+'uPSRpsr@™NÊ#9ÀìLogParabolaPSR J1203-63?¡ó˜¡H¥æ?¦®à&ì‰ô?îàÆu´{â?¦®à&ì‰ô?±¸ì^ý*Q?Áñ.`»¡?íÈât Z¶?Áñ.`»¡?Õ°0T0®Ê?³¸åL©¢?å'çÕ稛?³¸åL©¢?̳‹­zw?¢õAÈι?èÓ"¡b?¢õAÈι?]hEÒZÊä?e˜VX;RT?ïñKÝ#12?e˜VX;RT?F¤vŽÉÿ?©Ûa;äoœ?ï'ånj}?©Ûa;äoœ?Ÿ:ìÉS?±ÔàÓ¦?ëX1Dú
«?±ÔàÓ¦?¡oð³â?ŠÅC¥øöÂ?îéôéî¾?ŠÅC¥øöÂPSR3FGL J1204.0+1144@pŒy¿ß~€@QÀ»À5ÖÀ9°ÙQÀ;›¢ø½ì_¿ÒR¢v?«@%²A±%?þ	'€J¾¿çVöو'¿ÖßŠ§ä5¿×tæY1¿àœ²ßwªAGNbll@«¯ƒ{J#PowerLaw1RXS J120413.0+114549?ïÿB<)jÌ?sÀ*r?¸~«_u)?sÀ*r?ïã|¤ôÊ?€˜û:#·r?lƒZØ[¨Ë?€˜û:#·r?ïçmr§Åà?pHttˆ?h'eø?pHttˆ?ïüÒ
æ?)Ìå??ñ霌à?)Ìå?ïþ˜mc?#:4¼ Ô?'ù×.*q?#:4¼ Ô?ï_&ŒdZ{?¨ª¨Å?".p ?¨ª¨Å?ïê)É÷Ó?jp͐(Æ?eÖ6¹í¥t?jp͐(Æ?ï×N扨?kaăƒ?tXGÏÖ?kaăƒAGN3FGL J1204.3-0708@q­µ?|í'@Jño`
+ÓÀ9böo]†À;BöÕ®?×ýµ(/@ý4XÍ °?ýÇz Z(¿å0–Ý@|¿ÓP–ñH­¿Ô(SÜ '¿âV[À+dïAGNbll@¦³Á [ÀPowerLaw1RXS J120417.0-070959?ïôŸèÏH
?Yÿ­yê5?VÀ.-5Õf?Yÿ­yê5?ïÌ‰Œlq?‡ªr"Mþ†?yù»';ãÆ?‡ªr"Mþ†?ïÄÄÔl­?{o©r3?}•¨üiš?{o©r3?øË>"?lFÁ1B€?‰Ù×/?lFÁ1B€?ïÔÑïã}?ywõ‡Ð?u—|ݵ[?ywõ‡Ð?©aÛ?¬'¼ð?¥®d²Ö-S?¬'¼ð?ïxXБ?Ž±è&Ú?ôþe%È?Ž±è&Ú?ìô.I®8§?£'Î9MM?¸^² GJ?£'Î9MMAGN3FGL J1205.4+0412@q5»à~í@P&3`<ÎÀ:.
¦L/ƒÀ;͒ûç2?œ9>ce@ ä}m"@!=ŸÈ²·¿ì/£sžD¿Éë17–«d¿î?`Ɯæ¿ïÿ¹‰¬š0AGNfsrq@ÒF
¦L0PowerLawMG1 J120448+0408?ïYùkÄÒ¶?žÎÎdz9Q?"ÀҀ†qJ?žÎÎdz9Q?ïÊôNµ´q?Š¬5=?z…Ø›†ß{?Š¬5=?ëZþÔ0ï?©::þ"Ð?Á¾"¯<C?©::þ"Ð?ï9»=iè?€:%îaª
?˜È˜]úõ?€:%îaª
?ïNÓãu
? »ªæs?–<€!ÂU? »ªæs?ìí-é®k?Â&zÜԀ?¸–´Du
?Â&zÜԀ?éó×Á•Ù?³ŠÉÞ`?È0£¸ù¨š?³ŠÉÞ`?ã,0/Ñ1"?ÀQnñƒ?Ù§Ÿ ]œØ?ÀQnñƒAGN3FGL J1205.8-2636@r'=ÀTïF@A"ÌÀ7"À9+v2ŒDÀ;v¢À‰Èk?ÒnKa49@}ýîØ»C@S.Ÿz¯¿ä[8€$'¨¿çÒlÁ<‡¿ç'"±UÖ¿à<|+AGNfsrq@…ŽSÃa@PowerLawPKS 1203-26?ïÿipm6 ?³Ûè_?ÑîBà][?³Ûè_?ïÑž5Š¦?Š'–qñß×?w°èªHÊ?Š'–qñß×?ïÒ¦ÔHIÎ?xÒPoY)<?v¬•þ70¡?xÒPoY)<?ïè¥yÄ	?LnŠ+©?gâZÈ4vÿ?LnŠ+©?ïþ¡‹€|<?)´:êÉÀ?%çJdß»?)´:êÉÀ?îûúÆ@|Ù?ªâ§dêW¦? @S™d}t?ªâ§dêW¦?ï´ÕÁÙÎ?"RKó½·?'ʏš
,}?"RKó½·?îõ°M\¡Ž?'¬>ʲ? ¤û*5ç ?'¬>ʲAGN3FGL J1207.2-5052@r}©ß—ª¬@&ÉÁ?ÐÐhÀ9É:qÀ;{ö?ŒÝÉ?õÛ£g"Îâ@gwñB"@#à ¼Ž?Üu@å£]¿×K".ùñ&¿åÂHù꽿îaÓZGAPSRpsr@—×è§æ›PowerLawPSR J1207-5050?¸´ñ	©2O?¸Ûrà{?ìéaÞÊÙ¶?¸Ûrà{?فËØÂ5?ËK¡º¶…õ?ã?žæ?ËK¡º¶…õ?àÍå‡ómº?¶ô
¸Y'?Þd4ð$Œ?¶ô
¸Y'?âlô¬é¿?©ÇØ	U
?Û&ú¦,ƒ?©ÇØ	U
?"Þ¸â©Ö?™FàÌúh=?ïa
9òÑ?™FàÌúh=?¿¨¤Wn/?Àª< ?ì
ëuR:?Àª< ?¸ÉnΈÇ?¬•½b
â?ìÿ†Ñüó—?¬•½b
â?Ät­å3©ƒ?¤VÔN֏µ?êâԆ³Ÿ?¤VÔN֏µMIXED3FGL J1207.6-4537@ro@OÂ@0Õ€ÐtøÀ:4\÷QÜÀ;´²$ªÚ?õ}h%-a@Gý™Heõ@æùÿ_ò¿ç5§«uª¿¯ÃO`Þ¿âyaÅÇÚ¿ïÿõ³¶YAGNbcu@›¼£PowerLawPMN J1207-4531?®°2?¹'ä‰,&?î¤÷#k?¹'ä‰,&?¼],xPk?Å	ßõÏ?ìtZpõòœ?Å	ßõÏ?àŒY'
µö?³Õêb‰âí?ÞçM±ä"?³Õêb‰âí?οæF	?¦5×6°?èOP;Æn~?¦5×6°?­ãi¦Ÿ¬ý?·3 /N»ê?î!Ée±'?·3 /N»ê?¤ÉRuÁîº?¶¥ ZH¹?î³j؈d4?¶¥ ZH¹?ÇáßñB?³YĽ?Ù7?ꈼo?³YĽ?Ù7? cŒîð¡?‰Mãø2bE?îþiÇÕ¦?‰Mãø2bEMIXED3FGL J1207.6-2232@r¸_.Q@C›ãø¶À9´ýµ¢äœÀ;Œ27Š±¿ád"†Ò@ñ3¼Æ@™@ ¦n¿â¦-QØöã¿éYA}h©¿éÜ ï'¯`¿ÛÉÀ¤õAGNbcu@…[•µsê³PowerLawNVSS J120738-223250?ïüÚÎ!œ?<ÍÄ:»»?9)Gµ´@?<ÍÄ:»»?ïÒ­sáœ?‹XgB²?v©s؝"?‹XgB²?ï§Á&?H¯?1}¤8™?†¶sp9?1}¤8™?ïû4ºØê¤?0§Ÿ?C-©*œ?0§Ÿ?ïñî'÷|	?__­ Ý?\#¯'–Nm?__­ Ý?ï3{ìÏ:?£ï˜LêÓ?™'l÷è?£ï˜LêÓ?îáòTW~?™Äy°ûí?¡àÚ·üC#?™Äy°ûí?ï€AѱŽ?†×ÚËQÈV?ï‹Œ½G‡?†×ÚËQÈVAGN3FGL J1208.2-7810c@rÊhŸÆÚEÀ.ùûg¿,À:7jÒñ²À; Ôký¿ó˜Õ¿9¼9@1<6½|@*A`y£¿èþv§kF¿ãOL÷¿ØuEWHw¿à©9c'»HAGNbcu@£+¶È´9XPowerLawPKS 1205-778 ?ïýüÎ$ï+?)ˆ0yQÓ?0Œý‰tç?)ˆ0yQÓ?ïÂJr'?3¶ïH€U?~ÚÆüþiº?3¶ïH€U?ïßL-b—?gw¦'æþ?pY¸\@0f?gw¦'æþ?ïÿuÿ¿?ŒzÕä÷?@èS?ŒzÕä÷?ïû©|™6P?@ñB—J¸?AZÛ/"?@ñB—J¸?îh0IžÚ?·¬ßž@?©úŠ+Z?·¬ßž@?ïÏë7ˆ:?yO°tV?x
d~KÔ?yO°tV?ïõö—ªÛ?Q5j"m"?TÐóIö?Q5j"m"AGN3FGL J1208.7+5442@`úMÓØ@N«"ßöu=À8rS±À;ÃÉfæ¾æ?çĝúZ\@{´+k>@X˜ÀUÆ¿äúÛùî÷x¿æá^‡IàÊ¿ç^Çζ0ÿ¿ïÿâóÍ3AGNfsrq@{ë;¸<óPowerLawTXS 1206+549?ïþÉG˜V4?!Lé±tŠ~?#kƒÀö?!Lé±tŠ~?ïà==*á^?ƒJÇï®Q?o»šs?ƒJÇï®Q?ï"Vr8½È?'=
¤ö¦?ŽêcqЎ	?'=
¤ö¦?ïúBçK ?2içÜ:–?F÷À'­?2içÜ:–?ïþ´íÌ»t?'9X^>@4?$±%Ýû?q?'9X^>@4?ï?1I	?•ˆ(ì´c?°?3­½¤?•ˆ(ì´c?ï|¯Y…"Ž?Œ^ÑpØ?jÔtø*?Œ^ÑpØ?ïë8Jý²Ñ?_õËo'ʤ?dÇ´Á´‡?_õËo'ʤAGN3FGL J1209.1-5224@r†o€Uûµ@#܅_û¾'À9ùS‰XÀ;Œ¿Ígý¿öGþ3¢ï@
PëTø@Òc`¢'!¿éË"'È¿ç‰N'«?´¿Ý9iMM¿äø"PŒàNOTHERspp@'i¯·éùPowerLaw?ïê]Ìt?¤ÖÓ·§À‡?e¢4"gx%?¤ÖÓ·§À‡?ïÄ6'6ë=?Šn`"+Œ?}ä¾ôX•5?Šn`"+Œ?ïϐF½1W?uï^!gf"?x7Ü©¦d~?uï^!gf"?ïÿœ´ÅÞ¶?`ò\ÌB?ÒÀ;cy?`ò\ÌB?ïóÑ|›Y?dýÞ
"?X]dÝû?dýÞ
"?î«|™iÚ ?´"£v/?¥H6h†w	?´"£v/?ïr:VNR?Œ•]»@4-?'®º]ŸÈ?Œ•]»@4-?ï÷"Ô:ªK?Mï&"u<}?PöWt­êE?Mï&"u<}AGN3FGL J1209.4+4119@bñàm"@RXfÀ(yœÀ:×YîˆßÀ;ÖEßÞ"¿÷ÁèW´›@SxW)²?ÿ2Àœ'È¿èѸ®Õ"¿á
+¥Rèä¿Ã7DԊB¿ãÏK4åCAGNbll@¤ª2-VPowerLawB3 1206+416?ïÿ"‰%?Ž¶&1?
ÜI	´?Ž¶&1?ïáj¿l¬?‡b£kÝý)?n•€7<q?‡b£kÝý)?ïðeÛH‡ü?bMµï]]?_4I«i(¤?bMµï]]?ïÿîŽØ9V>ÙÓ¶m'Á;>áq"ÛÁÑ>ÙÓ¶m'Á;?ïÿ"U ö?ük;#æu?
ê¿}d´û?ük;#æu?ïÊô@À?•Ê( <?Œ»
IÏä?•Ê( <?ïñHð ?fOõ¯¿?]oÛ·K³>?fOõ¯¿?ïÿ}Oa?"ã°@ùc?üô³.qc?"ã°@ùcAGN3FGL J1209.8+1810@oºèÀHZ@S9Y_í¦aÀ9gšA_EáÀ;¬ìµ `]?Ô¾t~
@ÐXAŠŽå@a>ÀZ"¶¿ÝF\ë¾T¿å¡•¹1±Ë¿çmP@Ê¿ãyU­lÆcAGNfsrq@ïTÞ~¥øPowerLawMG1 J120953+1809?ïÿ_0œš?3@mÁ??Â`´¼?3@mÁ??ïÛjÎTó?ŠBzñ/O?rJ˜ÿdªr?ŠBzñ/O?ïÒÚV^l®?vöŠîWú?v'Ôï¶$Í?vöŠîWú?ïüÀÌÓµ?!(¶VÓä™?9ù›`èÓâ?!(¶VÓä™?ïÿ1qù'Û?)«Øƒ­øÛ?ÑÄâÌÄÊ?)«Øƒ­øÛ?ïv=«Ô|?˜Ãï?'8J…p}þ?˜Ãï?ïm~O1¨?ŒÜ÷Hi?'P<0òa?ŒÜ÷Hi?ï鏴¤ž?\z'Òĕì?fpKÚ?\z'ÒĕìAGN3FGL J1212.2-6251@r§µŸôým¿Ôl(€/mßÀ7ʇJâ|aÀ9Äcôœ¯?ÀùÉ«ÁJŸ@Þao@ç v3¿àU¬9¯N7¿çF& 'Ó.¿é8¡Nè¿ãœ€w_OTHERspp@˜~($PowerLaw?Õæ"\#J?Ñ63´ž"æ?å½ÑîZø?Ñ63´ž"æ?ïSí—6¶?¯<k֒ÉF?•'MW37?¯<k֒ÉF?،Ž9"?¸i©øó'?ã¹¹|¸ã6?¸i©øó'?ïÎyœñ_K?d'%^Ëã?xÃ1Ÿ]ž"?d'%^Ëã?Ñó'ösK?Í¥ƒ>°·:?ç}7Æ[?Í¥ƒ>°·:?ë
»xo0?Æi6Øâ¸O?ÃÕC?£?Æi6Øâ¸O?Ü})ÓÛVJ?½Q²( vò?áÁkTÛ?½Q²( vò?íÈzK[Ú-?y"Œ0ÇÀ?±¼-¥!.›?y"Œ0ÇÀMIXED3FGL J1212.6+5135@aÍ߆ã´@PM`#UÀ:'tVéñ¡À<ù7Žâ†¿¨n<OÕä@Å´'Œ¶@‡gÿ˜§¿è–'þõ¿¿Ú€]Q®5¿æÍNî-MI¿ã:©xx¦tAGNbll@—;Í5¨PowerLaw1RXS J121301.8+512942?ïü¥jï?Q¨*6 ·??Z׀*5?Q¨*6 ·?ï᧼r?'±Ñ˜"Y?nèXoˆô
?'±Ñ˜"Y?ïºUX÷èÚ?uýö@ÀE?j©Í´u]?uýö@ÀE?ïí¼¾â©X?K76®2Ð?bCA·À?K76®2Ð?ïÝj¡çú?sÏ:'±s¯?q@J̘¦«?sÏ:'±s¯?ïA§lëæ˜?¡†T«À	?—Ë`Ë^ó?¡†T«À	?ïž$ÔÜÍ?˜Sž-À?œ¬;`<ül?˜Sž-À?î'G!/X?˜lJg=?£T;Š}n?˜lJg=AGN3FGL J1213.1-2619@rE̟¶M@Aád ;ëÀ:1û9ÈÀ;¢þ‡Yûõ¿ì‹›óÄ{@`•™¯¾õ?þ.Ԟþ2u¿ÞµÁ"I«ñ¿ê¢%ùR«¿Ò‡¥; ?‡ÜèñÜAGNbll@±wÝ/Ÿ¾PowerLawRBS 1080?ïÿ+èá+? ‰sî¿ø*?ƒ<Lb? ‰sî¿ø*?ïÝ(®0:Â?'cB¬7?qk¨Îuƒb?'cB¬7?ïÏEüD?€‹N{ƒÇ?x]á $=?€‹N{ƒÇ?ïÿåÕv-s>ßAÛ¹J{Ú>ê*ؔ@>ßAÛ¹J{Ú?ïÿ9ùöу?ç6šÞø?ÀǦxºÁ?ç6šÞø?ïA1\)²½?¤Vz?—ÙÔ|v[?¤Vz?ïÓ^Ñ
ç?{°ìDZ?vP—›µL+?{°ìDZ?ïþÖЏWª?"êcæ£Ef?"'û©õ{?"êcæ£EfAGN3FGL J1213.7+1306@pί€Uûµ@R[¢Àh¡À9¦¦J'RÀ;ÁžÊ[…?îâä]&£@r°¹Æµ±@([À6ã¿ãœýd¢Êx¿åݙíÁ'í¿ëÉV~D‡¿ï÷c"ã©AGNfsrq@'ãIº^5PowerLaw4C +13.46?î2*ßtÀ?­ÓyÔ?¬ÝR+>ý?­ÓyÔ?༻ªŒÖ?ÎU»{'?ކˆªÞæU?ÎU»{'?îUF? Šxòã•o?¯ÏÊ«zæ¨? Šxòã•o?àoQjú?ª©Ü–Êo?ß!]+îà?ª©Ü–Êo?çŽ?sæà'?Æÿx®ð÷W?Ðã2?²?Æÿx®ð÷W?ÌJ&ù¶\?Ð_…rVoß?èíx¶A'i?Ð_…rVoß?èçV¥Ëx†?¸_bdä	?Ìb¥hÒç?¸_bdä	?©"Â)‰$ý?Šè¬ukj?îmÓÝY¯@?Šè¬ukjMIXED3FGL J1214.0-6236@rªI`0Â@¿ª×'?á
À7Öå•ñnmÀ9Õܨ#$?÷Nu»€Ê@>:\È-?þ¿Ü™žw$¿º}bVa`˜¿ãÜ[ýVØ¿å%±Ím¿ézØC""OTHERspp@¡oLogParabola?œèl<H˜'?©C'HµŸ‹?=æÁ|?©C'HµŸ‹?ڂ'wÍ}2?È*†vb?⾶ÄAg?È*†vb?ҘaÚªIÚ?¶êõK®ð'?æ³ÏªÛ?¶êõK®ð'?ãå^Ä»?¦öJ¡‡ò?Ø5Côv‰õ?¦öJ¡‡ò?g<W"Û-?nd('?ïèé@3T?nd('?­ª­UG¶÷?±lü¶•
?î%U*±?±lü¶•
?ºÅ8êéS§?³à‡håRÈ?ì§Xâ¢Õ‹?³à‡håRÈ?Ê©ÏU×ç¢?©Z^ÙõÂI?éUŒ*Š?©Z^ÙõÂIMIXED3FGL J1215.0+5002@a,ô!-w@Pƒ¾`"‡À9þ1Ýȝ"À;ÔÇýZ3R?Ô¶G5"ØS@RÙþ
·y?þ¶
 r~?ïIJá$É¿çoO ž¿ÁTªYãÔ¯¿åѱ'­AGNbll@¥Ë(e"¯OPowerLawNVSS J121500+500216?ïÿjœw^?;OÄX^?¬ECt?;OÄX^?ïؕâø)¿?"zEÜ">:?sµx<tt?"zEÜ">:?ïâRŸ°¬?laçÔJ§'?m­æŠê{s?laçÔJ§'?ï°¡÷A*?k±@;ó¸×?ƒ×'t?k±@;ó¸×?ïþ§ÑÑՆ?$1½í¬Û\?%'æ¡mÇQ?$1½í¬Û\?ïõ[¬? ïçÖ~×j?!NSø|? ïçÖ~×j?ïÑ9SïÒ?xÍA¿ 'v?wvc9ÛJî?xÍA¿ 'v?îo¯Þ³Ü?›Ÿ"éiL?©‡`D?›Ÿ"éiLAGN3FGL J1215.1+1658@pW"_ôö@S4z?̞ªÀ9´`ÎvñÀ;Àh‹Ô¡?èRßúÅ:@Gt.©6@‡¼Ÿ®·¿Ð1Ƽ›¿å¹6²Ää¿é÷ÏM
WŠ¿äœGãˆ?AGNfsrq@…f€IRPowerLawTXS 1212+171?ïù|¶½ts?Lö"q!è©?J
%žs?Lö"q!è©?ïªË'õ¾3?0˜ÛóJ?…MBsU?0˜ÛóJ?ïS€à\™?=¼CÕ§C?•ãù"J?=¼CÕ§C?îr©á÷g'?‡Úªaçp?¨ÕaâATé?‡Úªaçp?ïίû¢è?zrTw Öä?x¨qêÑ4.?zrTw Öä?ì!QWû-w?žb)‹??¾õu@&"G?žb)‹??í¸2HIc?¤¡£¤ñw¸?²>m¿Od?¤¡£¤ñw¸?â9¥è~Ñd?½jSÓ3:·?ی´/]9?½jSÓ3:·AGN3FGL J1217.8+3007@g›îàóË>@TƒDàá6À7i1"·ºíÀ:®•­¤é?å^·üŽ¹õ@Qˆ®d×Æ?ÿ—v~·k¿àÉø՜޿àDOÌಢ¿ßÃ`uiA@¿áùùšzAGNbll@•@ži­BÄPowerLaw1ES 1215+303?ïþ÷Q…®«?ñI¦^­? ŠêÎRâû?ñI¦^­?ïà2ðÅ?…µWœ;bì?oÍëã?äG?…µWœ;bì?ïȾz¤‹æ?€ðS©¼!½?{ ÂÅdá?€ðS©¼!½?ïóë:(Î^?Byó?X)Œ³?Byó?ïýJ@jÿ'?8(à™Š"¼?5­û³ïRà?8(à™Š"¼?ïnûãæ™Ò?¡à˜;ú£?' ƒ|Mº?¡à˜;ú£?ï£ ÞiNÆ?³èÇ¡Œ$?‡7È^Í©?³èÇ¡Œ$?ïÎd¢¶h?q@qX?xÍþ¿ÒØ?q@qXAGN3FGL J1218.0-0029@qÖÿâ£Ï@N¢ŸÒ˜¿À9|Æ@Á'/À;sþ¨+¡?àÁ Á"—@··M^­Š@]a#Ü¿äóa£ý‡¿åjÊ!)xþ¿êGDŒ™Mf¿ÑºO­ÎkAGNbll@'-Gy¦µPowerLawPKS 1215-002?ïÿ#ñ?!b¢B,¤?»—8Gòk?!b¢B,¤?ïÛ<F'Ej?u6ñØAÄ?raÜÙª>Ï?u6ñØAÄ?ïÏÖo?ræü§w¹?xôþu'?ræü§w¹?ïðsâi°â?F‰EaԞb?_:ýã‹L?F‰EaԞb?ïý	ƒ¿ñ%?IðgxE?7³á˜º?IðgxE?ïØ©qJg?­§vǟ Ì?ŸDêصë?­§vǟ Ì?ï7º2sù?'
+I?™È»iNØ?'
+I?ïD´–[\Ù?o ³Ï†Ù?—im6L2Ø?o ³Ï†ÙAGN3FGL J1218.4-0121@qà|`Ÿ@N5æ`ɊÀ9hq¡›À;`qå©é?Þ0$ðˆ@RìéLà-@Á?zê,¿Úà'yõíá¿áVzšÖ»¿æùïã&¿Ö·µœb)sAGNbll@˜f­\ú¬ÚPowerLawPKS 1216-010?0ýWž?´\·à|?€þ›»'®Ž?´\·à|?ïҟëÔ`%?"͝N§O\?v°
1m?"͝N§O\?ïocߒ;?‹Ÿîw&?'"'2¾?‹Ÿîw&?ï¸	ÐӐ?fœäÐ@I?ý‹Ñmè?fœäÐ@I?ï›R¹u¾?'MÀ։	
?‰+y‡S¼ƒ?'MÀ։	
?îÁ;‡üŸ_?¬36Uù?£ìG|Æn?¬36Uù?í¾Ñ²Ûe?¢ù²*€@?²	rn­=Ù?¢ù²*€@?ìªò4pº?ªè+=?º¨o¾\z2?ªè+=AGN3FGL J1218.5+6912@_Ïÿ`Ï‰@GÑN¿ÓÀÀ:O…¯
À<îøp¿†¿e»_p_¯Ú@¡P&l@&îÿ|¢h¿ê³~ÁT¿çÚ:Þo®Ü¿ïª¦!ÅÖ¿ïí7©¬–AGNbcu@s†î¢
PowerLawNVSS J122044+690522?æÅcmHéå?Ûä×a™Í?Òu9%n,6?Ûä×a™Í?ïÏh&@AË?Í¬LÝP?xKìà¤?Í¬LÝP?ï
ú2FàJ?"¹ƒ@<?ž@¹±üŒº?"¹ƒ@<?ï"LxÝ ?q½Ë/_?ŠìáÓ	ËÝ?q½Ë/_?î[FNæ9}?¼Õkc#?ªK›T61?¼Õkc#?îlvmŀR?°œ3ßùè?©8™!Eß?°œ3ßùè?î¦ôˆJY?œN;ó\$?¥·|;ak?œN;ó\$?è#¯ÚΘ)?¸~3C-º?Ïq@"ÅŸ\?¸~3C-ºAGN3FGL J1218.8-4827@r•øŸƒ¾f@,•"d~À9—æuë>¨À;…ª8MNg?ÃA¡b2Fœ@ÅUmðžc@°zÿzŸ¿á»Â/Ý4Æ¿âR1ÙR¿ã-1ò&µ¿ïäšZAGNbcu@"$3g ù	PowerLawPMN J1219-4826?îøcÌX2Ç?¢Wû#(L? yÃ7é"?¢Wû#(L?ï¬Ú>­îC?pa%¯ž?"ÉpJ5›R?pa%¯ž?íd†à·îÍ?¢1RÁž"?´ÛÈøÈ?¢1RÁž"?ïg6íÜO?u}mZÆ?""^üD?u}mZÆ?ë_Cý…Ò<?¼Õ¢Ò[	Å?'ð	è·?¼Õ¢Ò[	Å?íY¬9?¿çkÎI‡?·?%8Äx³?¿çkÎI‡?ç뿗7È!?¸`AåŽËÆ?Ð(€Ño¾?¸`AåŽËÆ?éŽH¹})?°|á[‡â£?ÉÆßý^?°|á[‡â£AGN3FGL J1219.7-0314@qù€#¦Î@MWý`OÀ9ÆÀâ³¾ßÀ;–ÿ³©æ?䓒T3'†@Á!ý*ãƒ@Ÿ§Ð"¿Öyw8':¿ÞU#ÁXØè¿à'Ž:ô¿âߙ
AGNbll@¢ncS÷ÎÙPowerLaw1RXS J121946.0-031419?ïú=n~?Hñ©ˆ
ÿ'?G
E…_9?Hñ©ˆ
ÿ'?ïyÑcp¤?‹ƒÞ·Ôï»?Œ!‹ DŸ?‹ƒÞ·Ôï»?ï»û¾Ò¹ ?~'¯*RI†?<‹f?~'¯*RI†?î^]Z#?‰
ËT°O?®¼¾É?‰
ËT°O?ïÑø¤R@{?w—jFó?w­ó¼zm?w—jFó?é»´Ï*8?Äèþ&,"?É,ÃWƒ?Äèþ&,"?ï\|ÓÒê?Þd²ƒ¶³?"p~ìdÚ°?Þd²ƒ¶³?â|rh
–¨?¶?À½etÑ?Û/äÒ±?¶?À½etÑAGN3FGL J1220.2+3434@d^Õ•:@Sÿí ‹]À9à5"FK>À;éC¡É¿êÕõ7zÄ@`<O´X@oÿl\J¿áò¼:ƒ^š¿áËcÁ¤\¿äŠÝcÈÒA¿æàBÙL´AGNbll@"D|"µÝPowerLawGB2 1217+348?ïù"V	? õ+'?K»vK	M? õ+'?ïäýý霴?€m᥎ÿ¿?k-À¤>?€m᥎ÿ¿?ïͯe³¹?yøÏ!¢Oh?y(M1"@)?yøÏ!¢Oh?ïüc4Fb?/ø'vÇ?<æ[ê˜^Á?/ø'vÇ?ïô¹Šr+¹?`:—ý¡y·?VŒë\ý­?`:—ý¡y·?ïi²¨«§±?¡]˜ç‹ù?'ɪìB×î?¡]˜ç‹ù?ïˆè…K?*?ŒWñ@)?ÅÞ´m…?ŒWñ@)?ït;÷¡?"®•UòbÏ?ˆ¢ñ Ì?"®•UòbÏAGN3FGL J1220.2+7105@_¢ïÝëÙ@Fè|à%o%À9Œõ#-+²À<|Ñâ¶C?Ò@XXå@ {KÆÓ@²¾ aŸW¿äII0[Ï¿åÁc"&¿ê"x×Æꤿè[ki;¥AGNfsrq@…eŽ¾ß¤@PowerLawS5 1217+71?琉ŸeÐ?ºf°äÿ?†þÑGSþ?ºf°äÿ?ïà+ðQ?~*׌Fß]?oäñÂ1¶¯?~*׌Fß]?ïÏ+{¦6?|­oíF?x@j$ A(?|­oíF?ïöáô?8r]`z;R?Sþ>(«?8r]`z;R?ïÿZ~%ÊÀ??-'"/h?°4îåÆ7??-'"/h?ï=œý–-?£´Ê|Ž?˜L`IÏ~n?£´Ê|Ž?ﶁdw+Ž?'¯9®jh¬?'_¦ðK'a?'¯9®jh¬?<§{/?xö$6]¢?‡°Äó(p?xö$6]¢AGN3FGL J1221.3+3010@gKØ't@T¯ &5À7É©f–7À:ˆ'–9?ٌ0¡Ð@Zys3~?úèÀž@G?¦cMû¿Û(ó/sû¿ÎŸ5åÀ¿Ñk…ÎÐK÷AGNbll@±Ø<j~ùÛPowerLawPG 1218+304?ïþÒ@™è?!K£ÃêuT?"ß>×
½ã?!K£ÃêuT?ïப^*?'ßFÿÈ<?oQUÁ~>7?'ßFÿÈ<?î5ן±?žle)7w?¦ü¢ŠPr×?žle)7w?ïõÌØ5?B2ÌÚC¦?Uçî'Ŗ?B2ÌÚC¦?ïýœ…\K?<VsH6?7{ïQd?<VsH6?ïxë<Š±?˜ëä2?â˜sÑIc?˜ëä2?ï'þjS°×?eÅÆb_?‹€e]UZJ?eÅÆb_?ïÙQT¨Æ?p‰æ"B?s{×65?p‰æ"BAGN3FGL J1221.4+2814@i5ÛߏG0@TÑî¿Ñ;ÇÀ7ÍÜcBÅwÀ;#Pg ¡?ëäb''k'@Fö¬o4@@Ñ£@Œb$¿Þ"yt51¿â'î÷øŒ¿àܽýôY{¿åXlR¹‹RAGNbll@]ãø¶PowerLawW Comae?ïÿsB—Õ?
–™Z¬¤?—¦Ù$_9?
–™Z¬¤?ïãÙ看?€Ÿr
±LO?l&îcup?€Ÿr
±LO?ïß9ñ_ˏ?pTn1+1?pcG+<Œ?pTn1+1?ïÚ-Éøî$?XË'0,º?ré
Û?XË'0,º?ïþâ=nÂÎ?%¨å6	âï?!Ü$ʃY?%¨å6	âï?ïT›azª?§LéYÉ,?•lÐaµ?§LéYÉ,?ïÔuм›|?}ü=šî—ô?uņ5b?}ü=šî—ô?ï`NÒKõ?‡ c,2(•?"ö%¯¾©[?‡ c,2(•AGN3FGL J1222.4+0414@q͞?»×²@P…IÿþRÀ8Fˆ'
YÀ;I_ND0±?õ±Óšt¦@ôDÖÙZ@Aâ:È'÷¿åk´¿˜dn¿ê–î¼ê4D¿ìíâtåì?¿ÝÌùˆA­tAGNfsrq@p~üÚQLogParabola4C +04.42?ïþ^q>J'?(.l'üX?*èhº¹?(.l'üX?ïÌ¿²÷¨\?"7›"œâÖ?y &¥(›?"7›"œâÖ?Y?•
!%›n?œ­ïÏ̪•?•
!%›n?ïaÎÍ¿!O?~8U{™hÆ?"Æ&P²Ü?~8U{™hÆ?ïý|™dC?<ûtvÏBÄ?41Eøï?<ûtvÏBÄ?îM"0À?²'…bš?«'¼ó÷ð?²'…bš?ïO¸FzZ?˜G)2žû¾?¶óÁ¿?˜G)2žû¾?ì8/'€G?²-tläYÜ?¾>ƒoýÉ?²-tläYÜAGN3FGL J1222.7+8041@_rÞCí–@B,Ò?ÓT¦À9+ªëÑtÒÀ;Ç«ZŒ='?×ي)(H@áuÁ"I¬@HÿÚÁ,¿à½'i›ò¿æÔ/[¿áå(­b3¿ê¸ƒÑJ#ÔAGNbll@‹[À6âëPowerLawS5 1221+80?ïþ½åu²?Ìí¬?$!§G2ãà?Ìí¬?ïØ싌™4?'9•œ
Âd?s‰º6ó¶3?'9•œ
Âd?ï¸W™ç>µ?<÷p¡=?ê‰÷ä ?<÷p¡=?ﴋ7é•?eþSl‹†î?'Ý:bçRÍ?eþSl‹†î?ïþA‰2?4fR}3—¤?+çh2ŽèV?4fR}3—¤?îŠY‡}.Ì?µHn5?§Zg‹œ¯7?µHn5?ïDZO#K+?"sœ×R?—t¶·b¦?"sœ×R?í£Ñ¸¼A? fÖë5?²ár9BÓ? fÖë5AGN3FGL J1223.3-3028@r|˟ÛÒú@@‰`fr%À:vŽŒ]"À;¼ól|*?Âv¥´ì@
¼Œã¨±?þ/ƒáK‰ì¿ãšOˆ¿åüqЧͺ¿Ü
«±Ò©¿ÉW̵AGNbcu@´!qÿ.HéPowerLawNVSS J122337-303246?ïþÜ5dT­?SÿͨYn?"<¦"Eæ?SÿͨYn?ï֗Wä²6?'²0ßÞÜÌ?t´T•á.?'²0ßÞÜÌ?ï輝]Q?Uv]'©?gCb›Ï«"?Uv]'©?ïõ_dŒá?@[PQ9ªå?UAóªYã?@[PQ9ªå?ïý¶~ð?2ÉVº?2O)@½ º?2ÉVº?îäà×h(«?±ÚŽ·îbW?¡±òˆ¡ŽU?±ÚŽ·îbW?ï⪠ÇÃ?oÔ°x?mUßwuµ•?oÔ°x?ï…éT~Ä?†2|9ä?Ž…ªÝ
rû?†2|9äAGN3FGL J1224.5+4957@`¼ÿÚ@S@P¥é`êMÀ:=އà4À;á¼é)ú¥¿Â¥ô*]³@L¤sgUÐ@´¶ŸcÝö¿âµý¨ëNÌ¿ë'Éùkø¿Ó7"E5­ü¿ëôHÖAGNfsrq@Œ¯·éPowerLawSBS 1221+503?ïýá?¥?)ŽX@¡ßÀ?0ö÷¥.—?)ŽX@¡ßÀ?ïæ—ÙG{â?xúܒ+(?ih&¬%†!?xúܒ+(?鬒3H›"?|˯Mƒi?…³1H¶ù?|˯Mƒi?ïðÇvTM¾?F v‰:V?^qÖ35\?F v‰:V?ïÿ%³Y? !ÄåĶ?ûE/b·™? !ÄåĶ?ïcE";?šŒV/ϋ?"—O|û8?šŒV/ϋ?ï¸àÃñÿ.?].nOVf?ÇφÖ?].nOVf?ïvàOǤ«?…¹ç5çj?'#ö¢p"?…¹ç5çjAGN3FGL J1224.5+2436@m@ôŸM¡@Tܸ¿ÏŽHÀ9†_:øúRÀ;ˆ›†Ù£?μÛÙì+H@𪮔Óa?þ0é
ìî¿éŒT¼ð¶·¿Õ0yשÁý¿ÔûòÇ)¿ãπل@AAGNbll@¦¦Çy¦µPowerLawMS 1221.8+2452?ïþ.0êÙ}?%ýÜ}$×;?-ñ	ÖӅ?%ýÜ}$×;?ïâ}­Í$®?€¨%£Õ"?m'R`òn?€¨%£Õ"?ïá}—k¨+?mF3Ù]?n'h|ú}8?mF3Ù]?ïÏÛ"âl?]
5°µmÌ?xn‰véó?]
5°µmÌ?ïúËe…?Gc]'Ã>Á?GäÒíŸöH?Gc]'Ã>Á?ïHÖÄ®?®Ö̓`Z?žå*ÙËÍ?®Ö̓`Z?ïÔ6´$½Ø?zÃßUÃ?u䦝SÅ?zÃßUÃ?îc!Áü*?™êãéë?©Íãçà=\?™êãéëAGN3FGL J1224.6+4332@anýæOU@R-‹àôÀ9´Rb£cGÀ;ÿžÁ÷†µ¿àºñQ!ÁØ@­á­.¡Ô@]  Ö¿æh¨µì6¿è õ(¿Ž¿æW|ûBð¿ïÿ⾦™\AGNbll@}[sbb˧PowerLawB3 1222+438?ïþÅ<"?)^á´?B"?.£°,åd?)^á´?B"?ïá¹z=;?'îr"%?nôF°]ìG?'îr"%?ï¤äœ³e¯?¿‹u.uG?†ÆØ֖0K?¿‹u.uG?ïï_ä—á?MÍmC	A?` cg¿;?MÍmC	A?ïýòEq+?4ӛbçiÓ?0mÖ(£Î?4ӛbçiÓ?ï
ˆÉly?ªïx­ð¥?ž®ð¢í?ªïx­ð¥?ï˜èÊnÊ?‡8ÄdôÑ?‰Å͉s!Y?‡8ÄdôÑ?îˆäÍkûs?ž>JÅ&?§q³(daÏ?ž>JÅ&AGN3FGL J1224.6-8312@ráoŸËÀ4a¦¹Ù«À9zeÜÓ«
À;{ ù	kº?¹3ݕ+}@#ÏÃøõ@Ž_?«'"¿ä‰'å´g¿êj\´Ù2ƒ¿ãü¶Ôâm¿í|3FUAGNbcu@~€DÑ¢PowerLawPKS 1221-82?ïhs¦P"?´Åu	½$?'ñœP]Y…?´Åu	½$?ï®D%k@ã?'!¢Ý¨ Í?"nö©OO5?'!¢Ý¨ Í?î–)Dw£?—qH0Š%L?¦k½ìžÊ?—qH0Š%L?ﲏ•)?eÜýý]l¤?ƒyœ(¶Ì?eÜýý]l¤?8Ñ
?š†"*Û%?™|õ;Y\?š†"*Û%?íIKÅ?(¤?»yISAVÉ?µµ¡ÔNìå?»yISAVÉ?íe¡Iç)Å?©LC¤•W2?´Òõ°Æ±Ö?©LC¤•W2?ì´øà|-?¡g3Õ°?ºX8üö•?¡g3Õ°AGN3FGL J1224.9+2122@oáç_ö	Ý@TjV ŘÀ5û‰SÑ8lÀ:e~ƒ"×?ù»]¹™";@#šŽSz@ñcá¦Î‹¿á"ìÂû+Ÿ¿åOA
çIP¿äÔ]X†åô¿çH%p|ê·AGNFSRQ@s"'ÞÑ·LogParabola4C +21.35?ïúõÅûˆˆ?I}Ô Ì‹?D(çîƒÅ?I}Ô Ì‹?ï弍9Ží?VY£Û?jCr÷ërÎ?VY£Û?ï"¼Geçˆ?˜ÄCU.?›¨wÓs	?˜ÄCU.?ïÿÿPL§>˜\Hþ*.>qÐÏ!ñù>˜\Hþ*.?ïõ׆þÑ?U2©¡'Æ+?TPò:›?U2©¡'Æ+?ï4:²Œ?™"¨—%…?Œ²újt%?™"¨—%…?ï:CÉ¿Z?–×™C-]N?˜·†Âæê¼?–×™C-]N?ïÿÿµ_üH>'ª¹6h>'¥Áš¡¿ý>'ª¹6hAGN3FGL J1225.7-7314@rÐÛ«–òÀ$íG¾Ûr'À9á¢!þW‰À;s`c'¿ò©0
3à'@>}[ËWØ@y¬ÿ§ël?çöE€‰q¿ìãrÜÁ¿Àvö%$–|¿çã•&ÔfZAGNbcu@˜v%`A‰7PowerLawPMN J1225-7313?ïú@"Ñ?IÛó¨¦Z?G¦þàYí=?IÛó¨¦Z?ï¼é¹9?c"'~ný?€û•yM?c"'~ný?ï¯õñ*Çv?}ËÈ› Ê?"ƒ¤x‡?}ËÈ› Ê?ïÿr‡9£B?x˜ó— ?¯˜"ªì?x˜ó— ?ïðCÑÞPû?c,'RJ?_x\	¤š-?c,'RJ?î'
Çúç?ºãÔeÈ[Ï?®wß$\8?ºãÔeÈ[Ï?ï'ð'ßn?"¡ôö¦SÖ?­Áó®??"¡ôö¦SÖ?ïû[ÌÀž§?Aû¨©amè?BÍ²ðÁ•?Aû¨©amèAGN3FGL J1226.8+0638@qÝõ€í @Q,ڀ¶–À:ámmÁ¤À;·ÉjA½:¿ÔôU–¤6@
‹w+/®™?ù>ÎÇÏ¿í··pˆíê¿ßø…Š…Q?ʦ`;ÿàu¿ÕS{ìÏ:AGNbll@ÁcA&éxÕPowerLaw1RXS J122645.2+063906?ïþJÙ˖t?-]#°u¶?+Rf4v§7?-]#°u¶?ïÛQÛiô?…£ÑÖÌÕÜ?rsÖïîîh?…£ÑÖÌÕÜ?ï×ã÷N'?rQÌ>¼?tti‹ÃC?rQÌ>¼?ïü3WEa3?-ɳ@ϑ?>eF@¶ó1?-ɳ@ϑ?ïû0ŒúF?E4mõ/=?C<õÆ
Éÿ?E4mõ/=?ï)¨­®h?­y¢ÈV›?šÊïÊJ2ö?­y¢ÈV›?ï¾q"éO?'·=µí^$?€c·>ØôG?'·=µí^$?ïá÷Ɔo?n¹šß–?n9ñy¡?n¹šß–AGN3FGL J1226.9-1329@r]®@…+N@Hxwò
ÏÀ9.x,a‡ÚÀ;R½¿Ïæ?îƒÝy\&5@KŠó8œT?ÿ¹V  žñ¿ïþÞY‰€"?ïèÏ;*è%¿á"30¦]¿åY¬µç´AGNbll@£e–_Ø­¬PowerLawPMN J1226-1328?ïÛ —ºœI?pB&d&ž?r/´>Þ§‰?pB&d&ž?í×H?;ˆ?¶Ë'h'œ?±E¿ŽtA?¶Ë'h'œ?ïcWjõí-?0hwO?"•šc"w?0hwO?ëY¡òX¢ƒ?¥ý0Aç+?™x6uò?¥ý0Aç+?ï›PFzõ?‡°‡³ê³?‰+üg'
Ö?‡°‡³ê³?èOH(@?ËR÷Ù?ÎÂ߃]Âÿ?ËR÷Ù?í¨Z9‡`1?¥¢f·aæ?²½.1Ÿ<ú?¥¢f·aæ?ÜîvOxÊ?À/2¿è/K?áˆôDØC›?À/2¿è/KMIXED3FGL J1227.9-4854@r¯CÀ~à±@+"É¡Ÿ!™À7蠖ãÜ´À;ϹWf?ø‡¤Ò1æ'@Džïnã8@–5¶ñ¿âZˆKµØa¿äP¡KÐÊ¿çü?^Ã8¿êßÿ_PSRpsr@{Ïâb˧3LogParabolaPSR J1227-4853?í¶ß‰á?¼%LÞç?²I_3°ö?¼%LÞç?Î0yÿd=†?ɵw[+IÛ?èsá€&ðž?ɵw[+IÛ?ì·S¤þä?¬w'ê 2À?¿zEbØâ?¬w'ê 2À?×ÿ#"Ð?¯5üì¨?än=±w˜?¯5üì¨?ÙÀ¬Ç­Ë?Ó+¼%à²?ã©À)?Ó+¼%à²?±}¹zpÅ¡?»²Ap¸¤Í?íÐHбçL?»²Ap¸¤Í?߬ˆt-Nm?À]ÆÖNçÖ?à)»ÅéXÊ?À]ÆÖNçÖ?­¡æçw•Z?š‡`nñ'?î%ᑈ†ª?š‡`nñ'MIXED3FGL J1228.7+4857@`™¥ 8L@Pî‹î²ÑÀ9èûŒ3€À;©ÏŽH,¿¿Â–Lwg@á©Ë•ë@ë€z8Ö¿äVˆ: ¸1¿äS‰ëY]r¿í94?*jë?Ì9¿ãǪAGNfsrq@–u$Z¬PowerLawTXS 1226+492?ïþ?òšw÷?7ö-5fæ?,Ò=^zŽ?7ö-5fæ?ïäké¡Þ{?€	ŽbC˜?k":e"Í?€	ŽbC˜?ï¶öW›Ùv?ƒ+¦'N¤?'Bj ð¼q?ƒ+¦'N¤?ïÿTk^•.?	'š0Ì0?r˜ä-+ª?	'š0Ì0?ïùb…U??Wå{Ìw?Jw浇&??Wå{Ìw?ïs¶Ê=6¨?–ĐÿqXÁ?'‰&¯Â$þ?–ĐÿqXÁ?ïr¯ŸëB?—B¤lÜ?ž'ª'ûº?—B¤lÜ?ïð~®9lf?aãø­E\?_£ÚsÐ?aãø­E\AGN3FGL J1229.1+0202@r¨@[9â@Pr@#Ü~À6nç=À:Üš\78?ÿ£"¦%@!ñ@­DFV@Zâ"o¿å±*SrÁ¿é8÷(JL¿êjÏÃ2€l¿êw({Y\AGNFSRQ@n¾ò䎊LogParabola3C 273?ïòä%Phð?XË2«n ?Z7µ33E?XË2«n ?ïÙV&8Š?Ã́ºÈ?sTìý(.?Ã́ºÈ?íóifƒ?§;£!Gã?·Xd³…if?§;£!Gã?ïÿÁì‰Ì>ôp2š' ô>ÿ	æM'÷>ôp2š' ô?ïã¹J¹â?nÙäAÆd?lFµFp©?nÙäAÆd?ïdÏakn¨?¢À_Âb"'?"fÐÚ]
?¢À_Âb"'?í·e#'£©?£C•;r>?²DÖ吤9?£C•;r>?ïÿÝà'ɾ>ø=y澑´>ñ´=õ@>ø=y澑´AGN3FGL J1229.8-5305@rºm ‹]@#H>¿ÙI]À:;zç&ë&À;Žã©8?°V)bßO@5Ãm}†é@,àŸ©¿èohÚ£¾Ð¿ècVX.ª¿ÑÙ9x'ÙË¿à`Á`¥AGNbcu@£¢¢3œPowerLawAT20G J122939-530332?ïÿE±v@_?ÉúB©?IɎlº?ÉúB©?ï¹½—ê[Ã?õðÝ,©?šUU?õðÝ,©?ïé2©Ôþ?pí¦¸;f?fÍVmöÀ?pí¦¸;f?ïúÄmòe§?-՝Gó…©?DîGâÙI8?-՝Gó…©?ïÿÄöƒn?-ŸtÈ<h?gh¨¸«æ?-ŸtÈ<h?íæ³MþCE?»»çë>Ûf?°Êe1þÙ?»»çë>Ûf?ïç.ôñ??w ÑÇ2"?hûÑ"l†?w ÑÇ2"?ïßRIè›#?c:ûL½Ý?pVÛ%Š7?c:ûL½ÝAGN3FGL J1230.3+2519@mF`¢G@U;{ îÙÀ9PY´§<À;Ÿ"ËÜâÅ?é¬^U©]e@:ä1Bm8@âàK¯¬¿Ðad¸«'¿å9ýgIeO¿ã߃ÍnL¿æ-b†Ì§AGNbll@F†Â&€PowerLawON 246?ïÿ"ø´ ö?ÈF"8Þ÷?â0;_?ÈF"8Þ÷?ïÕ£@óvk?ƒâkÏÄ¿[?u._uVˆ?ƒâkÏÄ¿[?ïÎËM#|å?|&Sâ[š?xšY]g?|&Sâ[š?ïVi&þ5?u)c]ÀÎ?•2ÞøÏZ?u)c]ÀÎ?ïÿnJ5ƒE?'Î5QÇ?6¾X8%?'Î5QÇ?î¯é±MÚ?°æRRœÕÅ?¥dìÚ,ˆ?°æRRœÕÅ?ï¹ÇýHd?"]O(d?ŽlVß?"]O(d?ëGJcÈÊ?ªèkã•?Á¾âÖpÜÙ?ªèkã•AGN3FGL J1230.9+1224@q½lºËC@R ÂÀ®À8ô>A"/À;c‰ì}l<?½óg¥<@ôÖÂ@R`0lY¿Òð‰«öú"¿á/¬i0Š¿ßÝí3¨,¿éÅN>b¢AGNrdg@›Þ…‡"ݘPowerLawM 87?ï"—V¦Þ?"e§®î%?Šþ-Åäe?"e§®î%?ïÕ{Î?…1ŽQî³?u}BQ…m?…1ŽQî³?îÖlU53?ŸÈŸiÝ×F?§"™8ôÞÒ?ŸÈŸiÝ×F?ï‰äñÂá£?v
åÀ"}L?†Ã‹×ûY?v
åÀ"}L?í×]
¤k?²É²1³.Ö?±Ebª¤?²É²1³.Ö?î²vƒÙ­ ?±Us¬ý?¤Ø—À­X?±Us¬ý?꒖÷Š?²¤A¦. ¦?ŵ§ü!½Ú?²¤A¦. ¦?ꥹLMr?²ÜsU?ÅiÏþÊ:?²ÜsUAGN3FGL J1231.2-1411@rxž?»×²@H1ÀY!À6ÿcëaãJÀ:á\·ûe@	dŠ÷t@DETH?ûšÞ˜–?¯ñO8!"Š¿Ù|µ^C¿ãV^´ó¿í«Kô±S†PSRPSR@Œ¯×süPLExpCutoffPSR J1231-1411?FÚtˆ—?I<ÇJ*Lí?ïúIb¨u?I<ÇJ*Lí?¹­'ç&Gñ?Ǔ]2"®§?ìÊMÃ7?Ǔ]2"®§?³¢- {sß?¤ªQ²+4?틺[¹—Ä?¤ªQ²+4?1BT÷¢W?#°©O
Y?ïý×µoIJ?#°©O
Y?X(@ŸG¥?Sæ"â
?ïóëóê¯?Sæ"â
?©BÇ«—÷?¾"ùu2˜??îk߃wˆ?¾"ùu2˜??¾°>¥ñÛi?±é;?«4?ì)ø+Aē?±é;?«4?8¤ Œî?40Øú—?ïÿ¯»DM?40Øú—PSR3FGL J1231.5+6414@_ qÁ
{ê@J`»oÀ: 'oÿl\À<PœÐ…¿?×Ì°áù@2ugMA?ÿwß	»@¿¥' x'Û¿×PÈfØôp¿ç;Cɔš=?Æ4U-j,«AGNbll@¬=¾
í)PowerLawMS 1229.2+6430?ïÓ(ßZª?®ZöªB"‹?vkRæ/^?®ZöªB"‹?ïß¾â(~¤?€ëÜBÊõ?p =´?€ëÜBÊõ?ï4}>Uam?'¡°¥Šú¬?™pX3œp?'¡°¥Šú¬?ïëH±RP?V+iYB¸ù?d·NŽ
Â?V+iYB¸ù?ï/và²ù?¨ÝÐ@*Û?š#ðžXÞ?¨ÝÐ@*Û?î¹ÒDž?µ(HÆÞÅJ?¤n¢Ðóú˜?µ(HÆÞÅJ?íŸ8¿[—x?¦Ú/©ïZÊ?³:mÀ?¦Ú/©ïZÊ?îxo …lÍ?§Ió]&_?¨y
ûô¶(?§Ió]&_AGN3FGL J1231.7+2847@gÙü?O@UV™¦5À82~5ÅÀ;
3Ï:eW?ã쏪yÞ
@C¨×¥ý?ÿ-À"!¿ÞÁ¼š½ ¿àÞúvÔ¿Ý7ÁÉu¿ßÃt|9óAGNbll@˜ÄwKƧðPowerLawB2 1229+29?ïÿ®¬>ûÍQÅ¿«Ð?yÔþçôk>ûÍQÅ¿«Ð?ïâ¶X—ä?'ŠPÖ#9?mI§TGsë?'ŠPÖ#9?ïçp­ù3C?h5D˃?hR­4¦?h5D˃?ïó•ÆÐÆ?AYLk«		?XÕÂǔÄh?AYLk«		?ïÿNì;ï?&ß}·ÙT?"x£Úë¦?&ß}·ÙT?ïmΐ­rü?žlõdD?'F-ãrh™?žlõdD?ïéößx~Ÿ?pæUX_²?f	 ¯\ØS?pæUX_²?ïÊ f–¦º?qP‡1Ûô?zïÌÀ[O?qP‡1ÛôAGN3FGL J1231.8+1421@q¤˜ˆv\@St÷íÀ:,÷öFBÚÀ;¼ùS="¶ÀŽ_¡¦-|@4Ö8±Li@…=ÀªÕ¿âqõ!¿ä+t¡´è¿ÜŒBX•¿äҏ™AGNbll@¤šCþ\'PowerLawGB6 J1231+1421?ïÿ0.ÆçÛ?ÑDS•ë?ú(–§©?ÑDS•ë?ïâ;0؏ú?¢z
T?mÄÏeHþ"?¢z
T?ïè$T{µâ?iò‡<6÷j?gÛ«£æ†S?iò‡<6÷j?ïÿûlŒ4>Ãá"ÑVûÄ>ÂM$yÉT=>Ãá"ÑVûÄ?ïÿ,a?  ^Ñ8ð¡?}®JÔɏ?  ^Ñ8ð¡?ïsoŒ"2?£¬%ê¶6?''S–ã®?£¬%ê¶6?ïæ}Ò,¡ã?n'ò½¢n?i'-ñš¬}?n'ò½¢n?ïÿ9ÓO6¹?$sx£¾Cµ?Ő/Z(Õ?$sx£¾CµAGN3FGL J1233.7-0145@r]cÿï9@Nf­ _À9úö«ÃhÀ;{µò•´?ÙÝW^‹§@üsƒôl@ÅhpM›¿åÚ¯/û<Ä¿ã<A"<ɿ㖭gÆ|•¿ÒÏç&×AGNbll@"›Ïß;dZPowerLawNVSS J123341-014426?ïêü©š~Ø?c8KŸà`v?eV†}gÊ?c8KŸà`v?,ù"@G?Ž©Ènvß?€ÜÁ«Va?Ž©Ènvß?ïx~ò?‹™—Ni?þp&çG
?‹™—Ni?ïUf9xzC?~huÃOBW?•S8Ï8éª?~huÃOBW?ï¥" 2ÇË?‡§Ø"u³§?†·wïÞqP?‡§Ø"u³§?íW¢Jº†?¾}ÁnAH—?·ÍBìÎDÓ?¾}ÁnAH—?î‹úÈ﮵?Br'#»?§@Sr¼â©?Br'#»?ç@Aæ<&?¿ÒZUa?Ñ|3χµ?¿ÒZUaAGN3FGL J1233.9-5736@rÉf?šIÃ@½ËCòžÀ8ÊÅ­ÚÜÀ; Îô©‹¿ðØOÒ¦*¢@Aˆ£¨U@Pèß|ý­¿æ¢.§n¡¿ÞèžÞä
¿âÿÉjä¿ÝE?IR@AGNbcu@ÃÉîËûPowerLawAT20G J123407-573552?ïñEw®bT?Rç¿âAŸÑ?]uçóˆ'?Rç¿âAŸÑ?ï³ÔåŽÔ?ŽG›ô3?ƒ?
Õº'Ô?ŽG›ô3?頋S۟N?^Ž^Z±Û?…+‡È˜?^Ž^Z±Û?ïþµ€'?«Á˜i ¬?&ô©@ÈËu?«Á˜i ¬?ïÖkÁ?kµ¤+ئ?tôÊL­Ý?kµ¤+ئ?îq'ñœÌ?¼…'h·h?®øí}v—D?¼…'h·h?ï%ÁWp Ç?"ødóM(Î?›GÕ	dá4?"ødóM(Î?ïÞ:
<ïÊ?jÒKÚþw—?pâúÿĪ—?jÒKÚþw—AGN3FGL J1236.6+3901@a&°)(@Sm~ßÙïËÀ:~1«s¶±À<
M`Ûã?Ä¡‹Sc\ú@0"[—*@ï·¿ttœ¿îFK­—A>¿È:́ʿã—e{ž¡¿Ø2Ÿ,´¯AGNbll@‹UàA‰7LPowerLawRX J1236.4+3859?ïÿ"6Æ?Jûà6e0?ÇÛfZÛ?Jûà6e0?ïܬ;1ÚC?†Àƒêåúa?q©âЈ?†Àƒêåúa?ï­±d͛:?ÏÖßûž¶?""¦ÐÍv?ÏÖßûž¶?ïà´6햶?V!Úeÿ¶?oKÉ2²,?V!Úeÿ¶?ïý=³ÈL"?<Íäåsgü?6bÄZl?<Íäåsgü?ïîpû/?®Ì¦<c_U?Ÿ/Â+b5?®Ì¦<c_U?îòö=Ÿ?˜8F@Ì»ê? ß zù	?˜8F@Ì»ê?îwè-až?œGdò?¨±{r?œGdòAGN3FGL J1237.9+6258@_b^AÔ¶¦@K
q VL=À:Ƽj~ùÛÀ<+Š«ÀË¿È;Ki¤£'@% ¢!}~?ýb
Cœ¸¿ìُ&_K{¿Ù¨L·"«¿Ön°Ëu›¿ÔlZÚàaAGNbll@±Ò‡ü¹#£PowerLaw1H 1241+626?ïëH¹_æ"?l¡TÙ?d·F›úUÊ?l¡TÙ?ïàOP*B?€½.ƒ¾>?o°~ŽÙ}±?€½.ƒ¾>?ï;ô,.©ƒ?˜jT» Ûu?˜zxs ?˜jT» Ûu?ïóWØÎ?F:AHY?YÇPoDÆ?F:AHY?ïpeçp?•EJ²·¿ù?'ÿÓ[óuø?•EJ²·¿ù?îåÿ±%§Y?²Ô–C†?¡ ê5îm?²Ô–C†?îœ+UC?£ýë ÷|?¦=G'>¯Ô?£ýë ÷|?ï4bµ×½Â?"rê‹Ø?™s©A˜«Ò?"rê‹ØAGN3FGL J1238.2-1958@r«f?šIÃ@EcêßÝJÉÀ9¾RsjZèÀ;´'¾ÙÅ?ÖÍ25K*@)ìþñb-@ÊÀYY¿éå-¤Òï¿á©ÉÆÍ¿Þãµ¼ºÛß¿ë¿öAGNbcu@)ᰉ PowerLawPMN J1238-1959?ï†Áˆ©ä?‹=§?|p?ŽOÕœå?‹=§?|p?ï¹ q~aI?'€áhš†?·ã'¡[ç?'€áhš†?îåЍæKé?"\ÁqÛ×°?¡¢÷%
Ýq?"\ÁqÛ×°?ïk±·ÑÃ?rc›ùJÐ?'‰É"u£?rc›ùJÐ?íŽvpËó?²l‹Mmù?³ŒL~›¬è?²l‹Mmù?íõÅΒ?¶OÔ
܄?°SñÒÕJV?¶OÔ
܄?ìV¡VO6?«y)$·Q?½JõOU†M?«y)$·Q?êßj±yµ#?¬VIþD̵?ĂU:+u?¬VIþD̵AGN3FGL J1238.3-4543@rÈÇ`|Aš@1cÀ™¸£À9Îä¦f&À;©:}ªP¿ï™£ÒO)@|b¤dùª@9Ê?©¹!¿í¿:ÓI?¢‹ºÖ!¬š¿à'n¦`ý¿åÔórFfAGNbcu@e6E¡ÊÁPowerLawPMN J1238-4541?ïþ
9[Ë?&6*|(.e?/\q\:>?&6*|(.e?ïÎ&×/QQ?‹QÐB¨:?xì"G[ƒ?‹QÐB¨:?ïàyp
-?qŒÆ‹¸Úû?o†í›?qŒÆ‹¸Úû?ïÿ#	«‹›?'²¬×£_?žÍ¦2¤ƒ?'²¬×£_?ïùÄf™3?HÏÒ_6²÷?Hîeê[ôV?HÏÒ_6²÷?ï/¨€«û¶?§é'J~›•?š
ïó>?§é'J~›•?ïĎ¡‡¾j?ódfàøf?}¸¯8±/4?ódfàøf?ïóL»'?U3i¸Â?Ygâ?M?U3i¸ÂAGN3FGL J1239.4+0727@rc}sÉ@QˆfxÀ9½â¯ åÀ;§†_*2¿ñŽÑú‰ @j«Yàq@.Bß·7¿éÓì$<0™¿á@­åßuú¿åì''GK¿ã¤	"AGNbcu@ŸŠ	ÞPowerLawPKS 1236+077?ïøGŒAÓ?SՋ—3G?OºâŠp.?SՋ—3G?ïÜ7m³?‡HÀ›ãŒ1?qÀw%ÞN?‡HÀ›ãŒ1?ï©Wåo0?z!ÔÓÁ[?…ª–uŒo?z!ÔÓÁ[?ïþ'Ÿ¡'?eͺ­»ˆ?'×'»'ï³?eͺ­»ˆ?ï­Ûß©?ƒŸ,Çõ‡?~©m	ò?ƒŸ,Çõ‡?ïMQ¨¥a_?Ÿr"›ó?–UÊð{>?Ÿr"›ó?î"[lÀÑ? êŽ}×}G?§ºI3òî? êŽ}×}G?ïÌ5Lµ\»?yV£hÇ_?yåY¦Žx?yV£hÇ_AGN3FGL J1239.5+0443@rs‰ :2+@PÚqÿ÷œ"À7'Œö(/À;¢!'—ô?ûuëæmˆ@ŒIõl~.@í*#•‹¿ágï¨nô¿å¥9¤¿æfâN3Œ¿êîÀmvƒžAGNfsrq@zŽY_í¦aLogParabolaMG1 J123931+0443?ïʋÛQ00?w¨Ò>u4v?zºj¥¸#?w¨Ò>u4v?ïØ}€<?‡©òß{Î?sÁ@ªŸE?‡©òß{Î?í×ÆÅ­â?£¬6?±AÉׂò?£¬6?ï÷°Kjj5??š¬­›áY?PŸhñr&ñ??š¬­›áY?ï~	ê©Ex?‹oDô`@†?>®Fìý?‹oDô`@†?ï>mýޓ?¦Cñ·áÚÛ?˜2]£³É¨?¦Cñ·áÚÛ?í¼Ï1^¥?¦Y>Ά†#?·"½<Ø?¦Y>Ά†#?ïô°3[o?S‰¾i¹€_?Vޟîrz?S‰¾i¹€_AGN3FGL J1241.6-1456@r¶a_Ìr@Gíù?ò^WÀ:C5'Ì÷À;Ækš'Í¥?â'AêÂ<a@º¿-§Ù?ÿYÊÿ˜&'¿îhŽa'&?žGь
v¿Ôyµ€¸Í¿ãé<¾5AGNbll@§˜{¥ãSøPowerLawRX J1241.8-1455?ïý=w²‡?0|4,MK?6F+†@?0|4,MK?ï¡+mäVy?ŒsdW–µ|?‡µ$ƒzÅÚ?ŒsdW–µ|?ïÞ øü‰?dåŒíÔÑH?púom";†?dåŒíÔÑH?Ûèñ?ƒq?UÓã—?¤5rC7Ží?ƒq?UÓã—?ïô±0ѱ?Uß;)ðÁ?VŸëÍ\?Uß;)ðÁ?ëœ"ùR?ŽL..D?Á•¬ž¹?ŽL..D?ïÆ_ät½?y^3""?|þP5=—?y^3""?疬˜œ–?µ‡ ±á?ÐÒ¦ÏüÆÔ?µ‡ ±áAGN3FGL J1241.9+0639@r'øÿûÎB@QZýç!À:{õ[aO¦À;ÈÎX%[?áTr^÷Å@^wڂ?üÄþÍ%?Ìqƒ£Á™F¿ê'äjÎ*?¬`Ÿ…ŸoO¿×åï!z=AGNbll@¶OŽzáHPowerLaw1ES 1239+069?ïþ¦lC}·?%P…ÉVk?%™=©ºž?%P…ÉVk?ïÞf¼'Z?ªï"ßc?p̡ñˆŠ?ªï"ßc?ï×ÚÁúXC?r1N$Ò҈?tžéfÂÌ?r1N$Ò҈?ïãÅëÃCG?VÜwbS±?l:£pî?VÜwbS±?ïþã¨A¹?++š?hä?.¡Å¹w?++š?hä?ï®®K$?§3*ÚâÉ?ŸÐ
/^}?§3*ÚâÉ?ïÀ/jLŽ?€	|Žš"Ë?èJÕ,ìï?€	|Žš"Ë?ï–D'ér?ˆ—¾ö^?ŠnßN3¡?ˆ—¾ö^AGN3FGL J1243.1+3627@`¡aՈ]@T Æà#Á¦À8i§e47?À:ùP°ò{³?ËQcøšÓ@@쉫æ?üM$þçüÿ¿Ý£!%G?ã¿×¹O»¿ØZé[!ܿӕ¾ùiRAGNbll@£ÍOßPowerLawTon 116?ïü9hpE§?3o*&ߨî?>4º{@}>?3o*&ߨî?ïãmR
[E?€¥"@tÞ?l'®Ò¹?€¥"@tÞ?ïÊ ¸µœ?wÅ9§3ê¢?zïð
§²?wÅ9§3ê¢?ïèx­÷Ûª?R¨ˆd²ðú?g‡QÓêE×?R¨ˆd²ðú?ïñö¥ÁΠ?\8©²õïß?\´°Ñ…?\8©²õïß?ïQšÈ©ã¥?¡EÏ´?•Ì¦çSïh?¡EÏ´?ï´_ö.#?ƒi†ø?'è9P2çA?ƒi†ø?ï83ÄíI3?Ž2E=?˜ù‡Y¿Ó¯?Ž2E=AGN3FGL J1243.9-0217@r±µß덂@NDÿ΁ÙÀ:L}qDçÀ;Ð:FLëk¿Ç­Í‹Â&@t¿CLZ÷@|Ñ`…Pâ¿çùÄ­ù¿ÞÝD3[¿Ó½°"퐿ê"ìiSAGNbcu@œäZ6âëPowerLawPMN J1243-0218?ï´4Á'?¤<(^
G?'òùor?¤<(^
G?ïم­Üû!?ŽóJρéí?s=(ö¾?ŽóJρéí?ïçTk?•û ªÏ?Ÿü#*jÂ?•û ªÏ?ïðægÜé?EϜ`èÎQ?^30Ò•?EϜ`èÎQ?ïÅë¡Üù?âñgXt?}
vÀ?|?âñgXt?ïD¹÷6?­Ð0k™i?ž7hÚ±}@?­Ð0k™i?îD&#*R?£u&thD¨?«·
ž©Aæ?£u&thD¨?ïh¸¯Î(0?†¦ØÙ?'èê
1ê?†¦ØÙAGN3FGL J1244.1+1615@r\:¿¹¾Ó@SÀW_ÍÅñÀ:6—ºœH¡À;Úe€…¿þ˜óï{xq@fÚ`´Ø@i1€«Œ
¿å±‹I¹vH¿äú–wâJõ¿ã*0¯dÿ¿ïÿÔ¸àÕAGNbll@ŒAÁ [ÀPowerLawSDSS J124444.35+161621.7?ïøîúHÓ?Pè¬n‹ãs?LEˆÉˆaÈ?Pè¬n‹ãs?ïã¸ä¸{Ý?'¥óåUˆ?lG='À?'¥óåUˆ?ï2£	8³?ŽëpM3?™«žØ1¶?ŽëpM3?ïÿä}Ý?P>æõ<
'Ç_>ë'ïN>æõ<
'Ç_?ïû6¥/Ø?L¿Ø…"È?C'þ	‡,?L¿Ø…"È?ï}~nxŒ?•7gX%q?\p.ÁR~?•7gX%q?ît}C³Å%? ƒ¿chì9?¨¸+ÇWbª? ƒ¿chì9?ïûÇÈ<U'?B'þB™#·?@àÞØɲ?B'þB™#·AGN3FGL J1244.3-4955@rÜ7À*ýÛ@)ÛҁA³ÿÀ:vãŒ+óÀ;ŠW™¿Ã?†Š•'@o"9櫛@{ÿªÅ'¿ê¥¸·Ó&¿¿æ[±9'ó¿àÃùòþB¿ÞIî±##AGNbcu@ ÓTzáG®PowerLawSUMSS J124422-495422?ï⫎c°?­çÔÄu·Ó?mTq™Ñv?­çÔÄu·Ó?ïʋ·\×?'öz}B?zº|°°,?'öz}B?ïæE{¬–?kóýDŠ?iº"ðZ?kóýDŠ?ïøM°OØ?5g©4©ÄL?NÉ>•ö¹?5g©4©ÄL?ïý6Š^Eä?RS>'mV??6K®Š?6Æ?RS>'mV??îS¡cx±~?» #:[ŠY?ªÅéÅL(?» #:[ŠY?ïÓäP¢ö?|ωô«}?v
ח ¬ô?|ωô«}?ï¢9c#ú?zòõ¯/à?‡q§:«^?zòõ¯/àAGN3FGL J1244.8+5707@_. {5+@Mýþ +ïrÀ:PÃë|»=À<¸e6»~¿ØšËOkšz@(=}¥@½?fj¿å£éqè¿ß öÍ0 ¿è½)¼<ë¿¡X\|F'AGNbll@¡¢mÅÖ8†PowerLaw1RXS J124510.5+571020?ïüˆaê'?Cú½²?9£ÌËIJw?Cú½²?ïäØIn?æ=Mž²s?k'þ
ñâ?æ=Mž²s?烈×D?{ZÏK«3?†X>¿à(•?{ZÏK«3?ïû¤€tÑÛ?3Ô˜Kýa?Amþª·Ý?3Ô˜Kýa?ïëñˆC
?e$AL¬N?dwëµ¢d?e$AL¬N?ïT#	^<e?š'r½Œ¾?•{žÍY;e?š'r½Œ¾?ï¯*>[Ê?"×
ó|œ°?œÊ±UNÆ?"×
ó|œ°?ïlmá|S°?'CªÝ`Y6?'rCÓå%ü?'CªÝ`Y6AGN3FGL J1246.7-2547@rÙÈ¿Â"O@BˆÄ`Á
À6þBÍ*1À:Ï;+O9#?ûpF™ @"±M?@ŒL/Ùa†¿ànK¾´9¿ä"ö•Ú-š¿å˜©PŠ Ç¿é+=}[lÛAGNfsrq@vãJôðØELogParabolaPKS 1244-255?ïÚBµËî?u›q¤1?rÞ¥
ª[]?u›q¤1?ïÆ,t­7?™#䋰Lä?|éÅçºh¹?™#䋰Lä?î"-{…©Å?›f8šù?¦½(FÉ|±?›f8šù?ïó´«ÿÞÙ?EØñ=ӗ?X–§ÃÉ.
?EØñ=ӗ?"åÇ?†U>rlß?‡7F›Î[?†U>rlß?îé¿Ä??µd'ŒöA<?¡dÀÁá?µd'ŒöA<?ìÿ…Ÿø¿€?©ÙcÊ("?¸Òÿ^?©ÙcÊ("?ïï{¨'b?Zq<À#-?`"êÕö"?Zq<À#-AGN3FGL J1247.0+4421@_fwž™@R0Ÿíp±À:šF…öN¦À<^â
¦²?í¯2½T@7—›è~@wå¿·æa¿æ9Öi>ï¿ë¨6ýHs?»(8¥°K¿Ó7âÿÐAAGNbll@¤ãS&PowerLawRX J1246.9+4423?ïþ=ü›±?2EÑQ€?, @'£8?2EÑQ€?ïßVG'ï9?"×[ˋ?pTÜ:§ër?"×[ˋ?ïÏr•¸}N?x€VíA U?xFµ* Ï?x€VíA U?ï㉃»¥¢?YWuX®Ú)?lv|b–î?YWuX®Ú)?ïþEªÀD?6àh…îA?/‹¤_äR•?6àh…îA?ï6c?{§'? !®‡"?™3˜²…(? !®‡"?ï ûù
By?ˆƒC‡ba(?‡ÁÀÞý³?ˆƒC‡ba(?ï²"˜õô}?€É&hŒ=á?ƒwYµfÇ?€É&hŒ=áAGN3FGL J1248.0+5130@_Ž`€sX@PgGÿÞrÀ:"HÊt,ùÀ<­»§¿êç
`™P|@ç	ç5@N¸@xÁ¿ëiĦ¿Ò|ҒÎ=)¿â&|§­¿ç©	¦ƒAGNbll@œ¿ëíúDPowerLawRX J1248.4+5128?ïý¶n]øü?6ÈjkÉÚ?2LŒ½Á€¹?6ÈjkÉÚ?ïâÑEyÔ$?ƒg'"ƒO.?m.ºMÒD~?ƒg'"ƒO.?ïÝOT¸$Z?j~"QÿŠ?qXUœ^®Ù?j~"QÿŠ?ïþX €µ?.{Òc(?*uøÔ"×?.{Òc(?ïö2bJD?V×N£šä?Sś5ì5?V×N£šä?ïhŸìnþ?™)~Š'ÂI?'ìs×ûð?™)~Š'ÂI?ïÑÚ±D?‹îގxû«?Œ‰P?@Y?‹îގxû«?ïà%)6@?jý¦Å5X™?oÚý¿lg¶?jý¦Å5X™AGN3FGL J1248.2+5820@^îÊâ°@McC hÀ´À7Òæ±z`ïÀ:ÿÕHœQ?â"èç#~ú@µO{é/"?ÿ(«Àb±%¿Ü1\~†Ý¿ßԒ;ßÝ©¿Ý…9ÿïÓ§¿Ü½œóì zAGNbll@•ËÚ¹õY´PowerLawPG 1246+586?ïýJÒûÔ¼?2Ê
݁?5©h¡þ²æ?2Ê
݁?ïÛÁ½V?v[IPx·Ð?r|Ÿa?v[IPx·Ð?ïf`ìځ?"0ØoU=î?"3â{Láâ?"0ØoU=î?ïNLVù>£?€fH"ZsÌ?–6u$Gǐ?€fH"ZsÌ?ï÷°wùÙ?ZQ–$ãòÖ?PŸ"KR9?ZQ–$ãòÖ?î±eà{ø–?±ó¼W%Ô?¤é¡ôÐÚ ?±ó¼W%Ô?ï]wêÈ5c?•Ÿîæž?"Q¨±!'?•Ÿîæž?êø}L9?´¯èR0Æ¿?Ć
ÏŒ?´¯èR0Æ¿AGN3FGL J1249.7+3705@_6ÆÞvB|@Týß=À9³ªŠ'¥aÀ;m¤K¤CA?ñ-
¦®*@—üï)n?úx@HŸ¿ïÿÒ~p&?ïÿ#Ý"¿Çzß¿Û­KÄ	ëÍAGNbll@±ÅꟾvÉPowerLawRX J1249.8+3708?ïí ®ü?bï˜7D"ñ?b_ý9#ԛ?bï˜7D"ñ?ïEr"›Ÿr?¨üyįJp?—Q¯iuÃ?¨üyįJp?ïL,2°MÝ?'S÷Úi.?–zy°Õ|G?'S÷Úi.?î0%Ne‹?"Ö1þ¿^?¬ý«_"?"Ö1þ¿^?ïßÙIq?p=|pmÃ?p"_ÎÊ?p=|pmÃ?ìôN¹ÿô?À+þǬä?¸]Š0ÜF?À+þǬä?îÏq¯g-®?›¯!ÂÒ¶?£å Ú?›¯!ÂÒ¶?êF҇v×M?¶ì|Wø ?Æäµâ$¢Í?¶ì|Wø AGN3FGL J1250.5+0217@ræÀ]RÁ@PJ¹ßõž}À::¬¤8À;²I|JÔ:¿¿$b#ÐXŒ@Nò^@Ÿž¿ô!P¿äF+"Eӿ祐¾¤¿ÞmŸÌtÉg¿Û#Þb\§²AGNbll@"­³œ¾àPowerLawPKS 1247+025?ïþîinrh? ^ïÝô–ƒ?!fþê? ^ïÝô–ƒ?ïڂjS?ý5¤îµ?r¾Êô
?ý5¤îµ?ïáQ{ó–e?bùq 4 ?n®"F#
~?bùq 4 ?ïõ=JÒûÕ??‹ËŸ?U…jW??‹ËŸ?ïü?ñT
?Bh—{"M"?>vô6#¬?Bh—{"M"?ïkŸ5dç?¯ü¯ø…?Ÿ2Œ1'?¯ü¯ø…?²‰T¨?Š&¡Káø?ŠÒgù©ô?Š&¡Káø?ïp˜áãµG?…²ë¬xh?'ìãÁщ/?…²ë¬xhAGN3FGL J1251.0-0203@r뿀ß×@NhP`j£ãÀ9Ûs"u"*À;²7_ÞO?ÛdÚ¨¶ @&°™_^@ùf!È?í£Îxoê¿è±úŽ|¿æÆ÷ ¶¿æ¿Ê+€ÚAGNbcu@ö0O‹YPowerLawTXS 1248-017?ïÿq]CÀ?ì*,¶ß?ÔYfÿ?ì*,¶ß?ïБ\".˜?',ÈúŸÛ?w·QÝ
¼*?',ÈúŸÛ?ï˜þŸ37?ƒò
9֐È?‰Àyéa>E?ƒò
9֐È?ïá&`'™?Tªo ã?nÙùÆT˜?Tªo ã?ïþ÷¥F(·?$2´u¤…#? …ªàVßÃ?$2´u¤…#?ï4³=–'?¢†óvµ?™iŸv•m?¢†óvµ?讀¦+p?"½ˆ>Ûæy?œËL°aü?"½ˆ>Ûæy?ï*ZÍù?Œâ)B¶?š¯ÍùͪÑ?Œâ)B¶AGN3FGL J1251.3+1041@rî-?ž{@RcÒtwÀ:ä9ÐÜ&À;ÃSP	,Ï?ѧâõ$§!@ÿ™©ß¸@'‡?Ïε¿êiMk¿çõ'C‰¿×.FíØ¿¿áX•:íÅHAGNbll@Œ$›quŽ"PowerLaw1RXS J125117.4+103914?ïÿ–ÃìÝ?BÉÅ8ÿ3?
~‹ïÆS¹?BÉÅ8ÿ3?ïÖË?rËh?­kì3Ûª?tš`Zˆ³?­kì3Ûª?ïèçŸr2?q6ΤŠ/?gínL>?q6ΤŠ/?ïñÌ®nèÁ?A7êÊùyG?\f££_Íd?A7êÊùyG?ïÿ»C"Ük?KíHê…	?/¶íó?KíHê…	?ï?™B(:ÿ?¤ùEâÉt?˜×µÑ6(?¤ùEâÉt?ïÙ*Z5og?x«þòtN?sjÒövX;?x«þòtN?ï™S4Y?z&r>»™u?‰½+@¶Ù?z&r>»™uAGN3FGL J1253.2+5300@^"®ÀrKw@P9ßõž}À8U'ÙŒÀ:Û«8þNO?ôE!óé@µ¹	÷P?ûæÁšê|‹¿Ö×,>CÔã¿Þhvšò¾¿Þ}âw­¼¿ã8á…ÁuAGNbll@"¢'½<6LogParabolaS4 1250+53?ïÏÀ
'Ì	?wæs¼Ž.ã?xú§ì«?wæs¼Ž.ã?ît!€`ì?±,™ŸÄÞ?¨¿½ã®nF?±,™ŸÄÞ?ï)JŸ
œ¼?"ï••!;™?šÖ¬<̃?"ï••!;™?ëŒ7[`ú? cW~…Ü?ÁÏ"'|? cW~…Ü?ï vB&–?¢i…‹°þ?›ñ>še4?¢i…‹°þ?èÌkÌ_r4?É"Õډñ'?ÌÎP΂70?É"Õډñ'?ëÿ)kç¸>?¬1•Ÿ)O?ÀZPa?¬1•Ÿ)O?ßœEŠ<ž?¸ï™‰â?à|±Ý:á±?¸ï™‰âMIXED3FGL J1253.7+0327@sп "`@P•€	¥›À9o™YعjÀ;^}Vlô¿ñdt
Ãâî@–«†ñÌ?ýwý%	O¿ÐV>Zø¿ß-‡Ç#¿ã,tè$Ë¿Àº½mU»@AGNbll@ª³a$Ý/PowerLawMG1 J125348+0326?ïü²ž€ç¥?3oà9^ßc?:k—@¢?3oà9^ßc?ïáÉ£ç?€º½,#%?næäFÚ8ª?€º½,#%?ï×ÓX­L?s"»
Çø?tS£õùÑ?s"»
Çø?ïÿåãk—>â®Èá³ßí>êTcÿ^>â®Èá³ßí?ïújò½!^?Dî)Ês?FT6Ή<?Dî)Ês?ïXòòHÑ?¥_áa
ZB?"ᡶ—­æ?¥_áa
ZB?ï¤ü+_)[?ˆÜ&¿®ín?†ÀõæÕ>?ˆÜ&¿®ín?ïýüÑçÆ?1ƒQœVÞ?0qãžZ†?1ƒQœVÞAGN3FGL J1254.1-2203@rüÀ?ö@Dg_ !¸À9¶ôöºÀ;"žý†¨ü?ÖXâíþÿ-@¬ã £Îý@]€k_ʿݔûùúÇ ¿æ1Æ=³â¿ä~ùlóà¿à^¬
+AGNbcu@–|"µÝPowerLawNVSS J125422-220413?î{+ßWO?ÈîfQ»?¨MNÿvÖ?ÈîfQ»?ïÏ,C]€l?ŽŸDOüqÊ?xiÞ=R
ñ?ŽŸDOüqÊ?ï¡ÀßP)†?…mxtÅ?‡È(†¤?…mxtÅ?ï­µ¿¿¯?euÇ?"'¸š^è"?euÇ?ïsU²¹ü?¡ä'éEVá?'•I¯Ÿ¶?¡ä'éEVá?îH}ãŽ7ï?±rÃåõ?«x!ìå?±rÃåõ?íú'@rÈ?§rFŒ‰ï5?°+íþ!×?§rFŒ‰ï5?ì&Ó÷8†.?§Ú"ô°'d?¾É`F;΍?§Ú"ô°'dAGN3FGL J1254.1+6240@^™"ÿ‰;@K9R¿ÀtÐÀ:†T‡@сÀ<€­9‰?ً€/ÿæÄ@o5w±…?þo'ßì\?ïÛýž?µf¿»w?"e쪿â܇hGDÁ¿Öº›¡ŽªAGNbll@§öE¡ÊÁPowerLaw1RXS J125400.1+624303?ïü…GZ»?VC·Žì\?;ÕÄZX'Ò?VC·Žì\?ïÐL93ñ?‹º¹ÌU]É?wÙãZˆ¯¸?‹º¹ÌU]É?ï¹äDã‰Ó?€ü*C±–Í?†îмsI?€ü*C±–Í?ïÃñ8‰UÌ?e±ëƒÉß?~cÆSÙí?e±ëƒÉß?ïêŠáùb?g´*õ,F?eúu6ÃÍ~?g´*õ,F?ï'P¾Î ?¢EÀè2Æá?œ-µß6?¢EÀè2Æá?ï4Ö¥­gñ?—E™7
6?™e+H›3Ô?—E™7
6?îÚWh¶g?¢ŠG­mÕÔ?¯Z†ý›?¢ŠG­mÕÔAGN3FGL J1254.5+2210@sr>À¨@U?Ô ÄÿÀ9¹âÅ\–À;ªw"^?äxg¯*"B@
¹sólÉ­?ÿî_a9€Õ¿è	
£_I¿Äò}¼Õo¿Ý­HTúÑ¿âi°IsšAGNbll@¤5Èۋ¬qPowerLawTXS 1252+224?ïú#pƒ±â?EGžÑ.x?Gr=l-ÿG?EGžÑ.x?ï¦z¨	@h?ácɃ?†aVnUñ?ácɃ?ïÖMj¨%µ?pˆ¥Ë"?tÙJ‹ Ñ×?pˆ¥Ë"?îB® —Ø­?‹¥ùBYhg?«Õù*/?‹¥ùBYhg?ïàºzMÄ?jw•ô'£%?oE…âTãÐ?jw•ô'£%?ê¼Ê¬ó#à?ÇÚ~] fŠ?ÅÕL3p?ÇÚ~] fŠ?ïH¾ñÓÿ?‰¶l*y?ˆ­ÐFúœ[?‰¶l*y?ã%¸®²°l?¸è¹ñ¶²?Ù´Ž¢šŸ(?¸è¹ñ¶²AGN3FGL J1254.9-4423@rùŽ?þó'@2yMŸÆ…À:[®UéAÀ; þ"ÅõB?á¦Ä'6Т@
vêb^ïÐ@Žâà_{¼¿çlXç³ê¿êÀ긽¿ÓÓàò'¿ÄvÛ">ÝûAGNbll@¢Ú¬1PowerLawPKS 1252-441?ïþo¨ô\?%>¤Ô½n?)tƒÉL9?%>¤Ô½n?ïÉrÌj6?…Xò1 ¹}?{F™³˜ð?…Xò1 ¹}?ïÚ7£§±Ø?tx‰œÁž?rä. xh@?tx‰œÁž?ïåýãù—º?R:v³º{í?j÷Iþr?R:v³º{í?ïü'µìØÓ?=åxпèÎ?;rO {?=åxпèÎ?îø{?¼‹òdЩ?®Àvþ8R?¼‹òdЩ?ï¦A֗¯g?†8M{Wâ?†oŠkB2?†8M{Wâ?ïKT€ú€(?Œôð¹XT??–•oâgÈú?Œôð¹XT?AGN3FGL J1256.1-0547@s†_•'Í@L‡Ã¤àõÀ6'_Tú-XÀ:}Uü‹×9?üãv$˜G@ ¯X	"µ@WæÄÊ׿â[#&9"¿æ.>¦Ñ2¿åHסßZ»¿ç:àH!#AGNFSRQ@u_t}€^_LogParabola3C 279?ï÷^ë6´?PVÙx?QB)E ªy?PVÙx?ïÔìªÒjà?†ìµRV?u‰ª+§ò?†ìµRV?ï{#P«Ù?™¬†¨ë?Ÿp›Lð?™¬†¨ë?ïÿ‡3²×P? ÊHíp??3 ÀôU? ÊHíp??ïä 
éŠ?nÛO·òKí?k_ýÊ{MÑ?nÛO·òKí?ï8…:šŽ??°Uøì‹û?˜ïX°Ô!?°Uøì‹û?ï>|ž?˜O[z'£?œMø9Ò(?˜O[z'£?ïÿµ
Ø©?Ãv¿?Úö?¼š±d£—?Ãv¿?ÚöAGN3FGL J1256.1-5919@røœ fè@VàºÛ^À92ÃWÙéÀ;Üæ"*¿É}Y†.-@5Í.œu—@X`d¿ËSiè½'¿éñX±¶µ£¿ßÀýFùIê¿áy³¤rAGNbcu@˜¼ñ²•êPowerLawPMN J1256-5919?ïñªõŒ‰'?^VÀ&—?\ª]mì?^VÀ&—?%Ò³¨?"¦×g&ø	?‰š¶}"¦!?"¦×g&ø	?ïu÷ÄOÙ:?ˆBü#ÞsÂ?'AvØÇ?ˆBü#ÞsÂ?ïñ?ÐF÷-?E1 Ð6™?]€_^w?E1 Ð6™?ïʉÂû¬x?}ã?]Â?z»¡Æ+Ð?}ã?]Â?í'­'¸M0?ÀŒ§ÅΣ3?¶Â–Àó»ÿ?ÀŒ§ÅΣ3?îzÆõó6Ä?Ÿ›Û6s¹É?¨S¤</½?Ÿ›Û6s¹É?ï[£ß?"²
#¦j'?"‹ƒûNtÀ?"²
#¦j'AGN3FGL J1256.3-1146@s
…ߨq¤@I‰L߬£bÀ9—RMª­¾À;|ë Í¿Ÿñ|Êúç@Vô™špY?þƒ %"º¿ç³֎Ë¿Ô½Û Ø°¹¿â-ßÐúH¿ÄXPüXÅAGNbcu@¨u…¸QìPowerLawPMN J1256-1146?ïýè«¥Š¿?$CŽó¦y?0º¢U8l\?$CŽó¦y?ïÔôÚă?'†w
Ë?u…'¬bš?'†w
Ë?ïá˜Gg¦?k› [Úç+?nógã3?k› [Úç+?ïü%H ?*гҀÏ?>Õ»"Öjg?*гҀÏ?ïûF¯‰<w?=YïæÛ?BåAiÎ9O?=YïæÛ?ïA8>µÈN?£ýÆÈY~)?—Øø*þÄ1?£ýÆÈY~)?ï³qå~'+?ƒŠ€?ƒ#†"o"U?ƒŠ€?ïÑb—¾'å?o$]á<Zv?wN´;"+?o$]á<ZvAGN3FGL J1256.7+5328@^I' ÿT	@OÒŸá²7À9Ñk÷Ÿß.À;'l	=–d?®÷û¸hSá@šZ]n›@ë@UZ¥¿ãì…g]‡¿êBÔíÇ]¿ä[D,L1¿ïÿåV9%CAGNbcu@†"¯O
"PowerLawTXS 1254+538?ïþW04ót?/…"ßíßP?*Œþz.Tñ?/…"ßíßP?ïÖaÃ`߶?†ÛÅmoà‡?tÏ0£©?†ÛÅmoà‡?ïª'lD{?xÓ&C8Ìi?…v%^}N?xÓ&C8Ìi?ïÊ$‡&'ÿ?` "Le@Ç?zí¼Šû@?` "Le@Ç?ïþ
‡mr?7»CLj?/W‹>±Š?7»CLj?ïŸ%Žsº?§šÒá†9¸?ŸŒOéV®?§šÒá†9¸?ï†Qz	ö?‹£ÚìŽg?Žk¡s3§˜?‹£ÚìŽg?í'8|rº?¢%T~U ?³v?½Ô80?¢%T~U AGN3FGL J1256.9+3649@]×®6	@TUÀ%õ]À9 /ªèvÀ;Áڅ4?C%҄@¸'ô´@¡Ë`;)!¿Ývƒ¢êÙ±¿àÝN,çGU¿ãÇÔ©©Ì¿Ú"0žÙIˆAGNbll@—IÓݗö+PowerLaw1RXS J125716.0+364713?ïÿrsåÕÝ?ÊJ¦æ?±€ŠjÙ?ÊJ¦æ?ïâcò~ô?'PX{¢ÓÌ?môœÀ½?'PX{¢ÓÌ?ïí—í"dô?e£ò^éܳ?bh˜õãÿ?e£ò^éܳ?ïïºôåY?Fó,öi?`EW6î?Fó,öi?ïþ멗ú™?#'Å*ˆ_C?!EjN?²?#'Å*ˆ_C?ï5^^Z(k?¨Ò¢¢n!?™T46rÀ­?¨Ò¢¢n!?ïӝ¼¥?|ÜÊà%Q™?vt1<ze?|ÜÊà%Q™?ï= ´bj%?Œ¥FS©þÊ?˜Kéz'ó[?Œ¥FS©þÊAGN3FGL J1258.0+6120@^`Ú¾'œ@K─U$öÀ:ÒÎX%[À<C"]È23¿êó"Q'²C@
Ì\Xp"@ÅQ *­¿ïŒ ÈÊ?Ö¥™§±_^¿Úøj
›ö|¿ÚKàZÀFAGNbll@£B\(öPowerLawNVSS J125820+612049?ïÝÎ.÷C?‹jªÃ¸|?qèy9ž{?‹jªÃ¸|?ïãA­Á¼?"=N†jH?l¾Rg5Ø?"=N†jH?î]ÉGm?¢ [ QÔ?ª.·$?¢ [ QÔ?ïþÅVG­?!o­¦Qž?#ªœ£hãW?!o­¦Qž?ïÃÁ…#ž?…*l1£Þc?~r9þ"Ë?…*l1£Þc?ï)ù¶dÖn?ª"T"{‡?šÀÉ1­d6?ª"T"{‡?îQºÈÆáY?£ÃW¨z¸?ªäSs'êp?£ÃW¨z¸?ïì¹ö ³?^7+Çù?cF	G$k?^7+ÇùAGN3FGL J1258.1+3233@[±þë-
@U[íöéÀ9‡"¹À;ÄnŠ!V'À¸gÏ2f@€2t†@»ÓÿÆõ¿åsôwek¿éÂÒ¼¿¨¿âšâ™èŸ¿åL?ôŒ¯AGNfsrq@‰jr{²þÅPowerLawON 393?ïÿíD«D>Þ¶ëFšÏ	>â»~uy
P>Þ¶ëFšÏ	?ïål"0±?ƒß"¤'²?j"kíºß4?ƒß"¤'²?ïñ_å!?Vlò>à?\ź#?Vlò>à?ïÿÿr͎$>`'mk†>'­Á¨	"'>`'mk†?ïÿï2—Ó>âvlô9È>àÍ\cÇÙ>âvlô9È?5+Â?™Ÿ¾x€'7?ŽÑrªÀ©?™Ÿ¾x€'7?ïê-šåA?m$~mxéH?eæґ¿??m$~mxéH?ïÿónÇx>áN÷t¸DŸ>Ùãð×ÿ>áN÷t¸DŸAGN3FGL J1258.6-1800@sY_í¦a@FjÍØã\À8•ÜJRÀ;wU·Ây?挆`#M¯@
ÜæöC¿@'eÿ¹3=¿älŸædοæ¦(c©ü¿ä¾²¢v"c¿ê–ón¢AGNfsrq@j¦µ(PowerLawPKS B1256-177?ïûÚæãE×?AÌ3ëãÇÒ?@"dy?AÌ3ëãÇÒ?ïÙY£'õC?…fúé?sS.1þg?…fúé?ï¶p‡|‹—?v>»gÊó?'cÞ,3Ð=?v>»gÊó?ïð
M踈?C2žo5¨?_ådP?C2žo5¨?ïý^P©vî?4¶£ÀkÌ©?5
yžhš?4¶£ÀkÌ©?îðëg†ù?²Á'"¢í^? ñI†kEr?²Á'"¢í^?ïeSr݆ó?ò=˜N?"U'«.Y"?ò=˜N?﷙=N·?s!oQt¤[?'Ÿ³"?s!oQt¤[AGN3FGL J1258.7-2219@s£¿ø¨ô@DAMå"mÀ8®ºŸ¹À;9&º~ìo?íËùÁS-@Ÿ=⎪þ@¶?Ÿ¨&z¿ã¼²ÕÍø¿äº1"X¿çuJ%NT]¿åB!´ÊfZAGNfsrq@lqø .PowerLawPKS 1256-220?ïýÙíû#U?/Ío2"J?10'	e0¤?/Ío2"J?ïÆ2õ~Oo?˜ÚJ'+?|æ…R¶@y?˜ÚJ'+?ﶣ>¢ÁÐ?|ä9GüÄ?'W0^†¹é?|ä9GüÄ?ï£uõigç?bçÆ|Áf¦?‡"'©¢$?bçÆ|Áf¦?ïúS­L?DËrV~ڋ?F±L¦1š?DËrV~ڋ?îÍh"³î?° ô(ß±Ò?£)v¼Œó?° ô(ß±Ò?ïì§f>?–hn®}d+?Ÿ¢kX÷ë?–hn®}d+?íÈmQ½?š6€[	Yÿ?±¼•r…"?š6€[	YÿAGN3FGL J1258.7+5137@^¬Óª7@P]‡ qäÀ:±äþú2À<Й
'¡¿þz5
(¯@
¯¼{F@E$¿ÒéG¿¾²lƟ-¥¿æ1±3ÐMF¿æPöñ5Õ¿Æuyv/ÿoAGNbcu@ 'ƒn˜PowerLawNVSS J125825+514225?ïùbg(X9?tèêµw
?Jvd1ºNÉ?tèêµw
?ïæ'
˜¤?#Ò§1#»?inõT?#Ò§1#»?ïuÄÔʋï?Š—·RxY?'Gedö´.?Š—·RxY?ïÿûñ{‹>Áhºs¥ÛÞ>ӝ)ïN>Áhºs¥ÛÞ?ïâã™0×Ó?yJ(S-,?mfüƒÂ?yJ(S-,?ïgªN¦3ä?©…'ÊÁ§?"
¶)µv?©…'ÊÁ§?î_4ΓÌP?£´ž¸ÕX"?ª³/†?£´ž¸ÕX"?ïÿ5Ç&—?$݊ÆÎl?G"ՋA?$݊ÆÎlAGN3FGL J1259.0-2310@swß (@CÓÒòäÀ9·ŸŒ¨À;€Kµàø?äôÑp@§ԖoÄ@:‰à>¿¿Ö€ºÈñÔw¿èS$Ê\&"¿µük­Ålþ¿ãM—"þ÷AGNbcu@¦*{À6ãPowerLawPKS B1256-229?ïýØst?7×~dq?7)=~BY?7×~dq?ï·´J±h?–ÿÁ'
q>?'íLÜíû?–ÿÁ'
q>?ïÖêx´G?sö×Í-Þ?tŠùÍô°?sö×Í-Þ?ï«Ô&)Ø?q'¤ċ?
…r£¿?q'¤ċ?ïôd#ý…?T¾ºé]Æ?W7·ÔN•Ÿ?T¾ºé]Æ?íÉ Ÿ °é?µô;à)A?±¶ûÖ_´?µô;à)A?梨ækÑ­?‡b䎥î¾?†FZ¼Àä?‡b䎥î¾?í§ØFRŸµ?¡‰l._5†?²Á=ÌýØ?¡‰l._5†AGN3FGL J1259.8-3749@s/hی@9$;I'À9¢Ö(–!?À;ŸÛÔ§Œ¡?ÙfJ`»@où¡A-È@îø 7­ì¿ê	‰…i%¿ßÔ«±|ÂÒ¿á&ŒÓ|X/¿Ý†ª,þ'AGNbcu@"Œº^5?}PowerLawNVSS J125949-374856?ïúm%ꗰ?GBÁ˜~£?FKi"#—?GBÁ˜~£?ïÁ°s(?Š;™Yw?'Æ4+§‹?Š;™Yw?ïÖ`2ßj"?p&7‹ØFñ?tÏ愜Bÿ?p&7‹ØFñ?ïž*ÅÑZü?hƒ ¹i‡Ê?ˆuN}êÑ?hƒ ¹i‡Ê?ïÓLE}ã†?zž£j8
$?vYÝ[Û1
?zž£j8
$?í—¥Ñz?¸æºÃ6«K?³GÒP?¸æºÃ6«K?ï2Ÿ¶g—?•Jx÷Ÿ?™¬¢©!?•Jx÷Ÿ?ëç°ådÿ?¦«QØî™?Àa<jl?¦«QØî™AGN3FGL J1300.2+1416@s‡‹À]RÁ@S?ßеÀ9L#Ü~¸À;®d¾£?ÞXìd[Ž
@Œ+·ü1@×:€.Ž‰¿ê+°#"5¿ê©ó~'W0¿äïÉíÛvo¿ïùé÷¢AGNfsrq@u¢¢œwškPowerLawOW 197?ïõ8OÁx?TH< l?U`¹ˆâ9?TH< l?ïÍtkè?~è˜_#ÓL?ysÅÀÛ$C?~è˜_#ÓL?ïTô2¹³?Š•ï['"?•ay±`¤t?Š•ï['"?ï
ÿòáUè?'(ç1×X?ž ª´zð?'(ç1×X?ï÷䉊Ù?\͙Ra;?P7à҆èQ?\͙Ra;?íf®¶ÈdÄ?½ƒâ?ó?´ÊŠHàòÞ?½ƒâ?ó?ï5ÙªšŒ¢?"Ô÷ñŽ"?™Dʬ®k°?"Ô÷ñŽ"?çUý+Ô?·†'" &?ÑT¨WïÍ?·†'" &AGN3FGL J1301.6+0832@smD@lÚ@QÐGßþùÀ9D`Þg)À;¨âøˆ<z?î…У_ÚË@
ÙRl3"è@@dÊ¿àWe¿äºH«ÿ4¿æE3w•|˜¿ïÿïʆT PSRPSR@‡ì
Oß;dPowerLawPSR J1301+0833?çé؍dö?ɚa"n(?Ð,Nå7Ê?ɚa"n(?à'¢"‡•?ÐD©($P?ÞÚº×èðÖ?ÐD©($P?ëxä‰=<2?«oŠÂà;Ÿ?ÂmÛ9?«oŠÂà;Ÿ?Þ­×ÉÕ÷n?®³Ë×?à©I?®³Ë×?ãçOÙËҖ?ÐR¨ú	ÆÓ?Ø1`LhZÕ?ÐR¨ú	ÆÓ?Ð8h1ÎN?Ó¾°ÕJ?çãËçt˜Ù?Ó¾°ÕJ?⢊·‡?»ËPö½Œ?ÛþºêñÄ?»ËPö½Œ?¦ÌfÎÕ¶a?8uéñ]Á?î"9"IžZ?8uéñ]ÁMIXED3FGL J1302.3-3259@s;?¦Þü@=ÓÝÿú÷ƒÀ94¹šûÀ;'h§‰Fe?ý7ùÁw"@
vêªÙ2?÷…«'	?ïúŠˆÏr¿×Ð.½§¿âwõq©¿í`ö0ã PSRPSR@–'Š#9ÀìPLExpCutoffPSR J1302-3258?l¯ôaó?‡Yvàòa?ïãPÜH?‡Yvàòa?·Oª}»™?ÃSž'ê½g?íö
çBM?ÃSž'ê½g?¾Q$Œ}/?¨&F…l?ì5Û}®pZ?¨&F…l?±?»`¹ŠB?'Nz_¸9|?íØ"
?'Nz_¸9|?U…Úk
*÷?T0<ýòµ?ïõ=ýU"?T0<ýòµ?§"EØ×f?¼åÓ©ŠÓ?î†Ë¢;ß?¼åÓ©ŠÓ?¤]6èåÖ?™­ø­BœF?îº/Œh6S?™­ø­BœF?€äÉ;Elñ?k
3@u/?ï¼lÚô­¼?k
3@u/PSR3FGL J1302.6+5748@]ÿò¾ÎÝH@M \ßÔçNÀ:…6ÍòfºÀ<$y'¼U†¿ª±›aþtP@;*Å{u@-_§°^¿ê¡:fпæÍ»
hÊÖ¿ÓØb<`-'¿Üº¯6*èAGNbcu@–+@·€4nPowerLawTXS 1300+580?ïÿ6h¿(—?0ö³.òþ#?2ä2^ìÞ?0ö³.òþ#?ïäP3k‰³?~Ô[¦âµ?k¯ÌY]?~Ô[¦âµ?ïß,Jᥢ?r¸<OÕ>?piÚy/¯,?r¸<OÕ>?ïù
Äv?3˜Á:mO?KÈï`'õ?3˜Á:mO?ïüÿ°'qè??±IøÑÜì?8z"1˜¶??±IøÑÜì?ïS1·¡Ü"?¥	Ú!µæ?•™ÉåCÆ?¥	Ú!µæ?ï"1  ?'‹Ýi3=?Žó¸ÎR?'‹Ýi3=?ïÃn¡¬?tìÞén"?~È®QË?tìÞén"AGN3FGL J1303.0-6312e@sÃ{á"¿Öâ:""•À8'£¥AÀ:NU\Rç.¿Ù™bìc@Æ_Ȓ€v?úDå)?ïú-Ç©­¿åhlÐ㳿â1¢4rÎ?Á!™h§^OTHERPWN@щXbNPowerLawHESS J1303-631?ìùÅ'§?˜ì›þ?¸1׍vôÊ?˜ì›þ?ïwZµ¶¹C?¨ºV:Â?'©NPA¢?¨ºV:Â?é4"LjO?µn]uüÜ_?Ë-²ÏºVÂ?µn]uüÜ_?ïÿFǏ¡?/ùh'Í?'FÂÆ?/ùh'Í?ë²¥%¶??Åå,ó†©?ÃÅ5ki'?Åå,ó†©?ìu5ŽN¯2?ÅD@8v¶b?¼VSŠ†p?ÅD@8v¶b?ë 7äÒ?±®tÞS|?ë#l¹?±®tÞS|?ïøÌý?KÚZ©Þ€?LÏóVÊ@f?KÚZ©Þ€AGN3FGL J1303.0+2435@uՍ@$³>@U—‹àôÀ8‰ñ…é¹À;m˜«]|?ëÒb?‡¡Â@»V†''@r±¿€3¿ØÁ'H¹Ï'¿âú¦ôÃXQ¿ãڔßÜ°+¿äNÆýTÿâAGNbll@Ž Àƒn˜PowerLawMG2 J130304+2434?ïÿUµ‹Š?ÓU‹Ìä
?IT>€e§?ÓU‹Ìä
?ïá‡Z8?€&^BéO3?náü®?¯ ?€&^BéO3?ï±í¸ÕŸ?'%[3v\Ð?ƒ"'ÖFë?'%[3v\Ð?ïûgâ½O?,vnÓû*m?B`t.l~?,vnÓû*m?ïÿéá§ó?¤³˜'8y?¢Æ̪(?¤³˜'8y?ïXñr7nÆ?¥-g~Áz?"áѵ¢‹F?¥-g~Áz?ïšÛý>?ŠVþmZ?‰xHó@¬?ŠVþmZ?ïðœ¹oÞñ?U¢Œ‡ºUp?^ƌËÍÛ?U¢Œ‡ºUpAGN3FGL J1303.7-4619@s~KZ@0ñ'lÀ9t.¦¸§À;ŒËÔHµ¿çƒÑ¡¦a@+‡ø[Ç@]à
Ü¿çhc'\ʗ¿ãÁöçÊÌd¿çfå\š=¿ç@>"iPAGNfsrq@Œ•e@ÌxêPowerLawPMN J1303-4621?ïú¡:Ã~?D-Ç%Pl?E{¼	–6Ð?D-Ç%Pl?ïÊńÆe?Œ‡üf­?z>
‰6?Œ‡üf­?ïŶÕ-ˆ=?y~&Ì"á?}$•y
J?y~&Ì"á?ïþ+~ôI?5:æÝE?-Nw9:TB?5:æÝE?ïì£Iú'¬?hv#Vöù?c\µÝüÛÂ?hv#Vöù?ï/kÿò,ò?§û‹Òƾ?š€)ý®?§û‹Òƾ?ï>rV‰¤"?"ìNwÅ?˜1µ)¤‡?"ìNwÅ?ïݛ²V1™?fÀ†ý¼'?q2&µú·ç?fÀ†ý¼'AGN3FGL J1304.2-2411@s*³ S\ž@CJà€øÀ9¤0íCÀ;yIoH?ê¸-ô¸Å@¶ì²Eb
?ÿPò@¤µ×?ÕPHÌfdR¿ØIµ‹g§¯¿âAÇÝÇp¿ÚØ/ßõ&;AGNbcu@¥ªµÂ\)PowerLawPMN J1304-2412?ïï%_5½?`#D½œ?`Ú ¨Š*ï?`#D½œ?ï¸(B"O-?…­(I?õïa€¾?…­(I?ï¨ÖÆJҌ?€~ƽÏ9?…ÊN\Q
?€~ƽÏ9?ï#6'??y Èþ.?>?›™;XÄ?y Èþ.?>?ïØnH)†Ù?lÍV€"e¦?sÈÛÓß;h?lÍV€"e¦?협ØkL»?²"5™¤]@?³;q=ït¤?²"5™¤]@?î›mH¼? =/%Ï?¨I,Z+9? =/%Ï?êgb%þ±?­á\ã?Æbwh;Ã?­á\ãAGN3FGL J1304.3-5535@s^¿¨÷Û@ö© JMVÀ9xþï^ÈÀ;-QîÊN?õC5Ú£@'Øì?Ùµ@'/ÀbY¿ßðë(ò+¿ì¤¯ÿ;_¿çJÒ6C3¿ÝßQ‹Û7kAGNbcu@Èh>BZîPowerLawPMN J1303-5540?îréÛÀ'?¦Xgæ'G?¨ÑbBFIÜ?¦Xgæ'G?æ‡…DøØ?Î>	ù~?ÓæðõvO?Î>	ù~?íÆY:Ùů?ŸÒÛèE9 ?±Í6(Ãß?ŸÒÛèE9 ?ê0ƒ|-"?§?†OPO?Ç=ó–Kw?§?†OPO?ë£	¿hØ~?ÀI1uN¥?ÁsÙ\ž?ÀI1uN¥?ÖQCG0?ÈU';a³'?ëk¯.3ù?ÈU';a³'?êŸ_܉ƒL?¬+*¹·è?ł€ÙòÐ?¬+*¹·è?Ö§Oˆ+?ÀRFɽù ?ä¬Xvõ»ë?ÀRFɽù MIXED3FGL J1304.3-4353@s[ߏG0@2逾À8D7guZÀ:Úá& %9?ä³i0Ü@D‹çTbƒ?þ…ÜiM¿àlõÈÞE¿Ù1Ídn¶ä¿ØÕN\j C¿à'Í2|AGNbll@¡»I^ž	PowerLaw1RXS J130421.2-435308?ïÿàóÔ?1Ý?ï½.HŽ¡?1Ý?ï¿KÙøë?ŒèÆÁC?€-<è??ŒèÆÁC?ïÕ,ü§×?uâs±?ui¶|c?uâs±?ïÌqáLiC?[—.dbo?yÇaZ'"?[—.dbo?ïý³£Ê¹¼?/fƟ=rÔ?2bãwýžA?/fƟ=rÔ?îÞL–Üzë?°Ñ_Æ~Ú?¢6"8T?°Ñ_Æ~Ú?ïÕÅÄ3»?~Wö6¥F?uv	Hz®?~Wö6¥F?ïºÂÖv;?ˆ2ÔÁøXM?ž(§¡Áœ?ˆ2ÔÁøXMAGN3FGL J1304.8-0338@sWÿŽÀù@M†ÿ ^¯¹À:ažõ!À;ʆ`ñ˜¿Ì$Ǟ±ÿ@1mÇXÅ@>€ vÿéìÝîœe¿Û©VÉmû9¿çñÊ8%"ì¿ÊÔ¾!¨
AGNfsrq@–Ù˜_÷PowerLawPKS 1302-035?ïüµ
–åh?<†Ç§»'Ø?:W©¶héÞ?<†Ç§»'Ø?ïܛÂ߁?ƒŸ­©¡ÇŒ?q²ú¯Ç£?ƒŸ­©¡ÇŒ?ï±¢Ú"'?€6—4ê€?ƒ¾×F›kf?€6—4ê€?ïÿ
ê?™[Rÿ\œ?ý¸Æh?™[Rÿ\œ?ïõš‰·,?\Ãog'<Á?TÊì1rçõ?\Ãog'<Á?ï-2ì"
?¨s(e«©²?šY®	L¶»?¨s(e«©²?ïÿږ9?•:ùÈzÏ÷?ž ²`G»?•:ùÈzÏ÷?ïñęޟ?VxŠýç?\vËÒŸ½?VxŠýçAGN3FGL J1304.9-2109@s2"@lÚ@DÍ0úŒ#À:7Ϗõ«éÀ;™S ' ?ќ®Ñ(@¥í¤ܘ@.ÜÿÊÐô?ïÚbð÷4¼¿ê.f›Ñ"l¿×¼<a/Dç¿æ2rgâ¤AGNbcu@£¦å`A‰7PowerLawPKS B1302-208?ïýšP–Ï?<?©¨€%(?3/-ý"´?<?©¨€%(?ï´4ð$Œ?'x
?ÊŒ?'òÃíXE*?'x
?ÊŒ?ïÀÆEbúe?xp?/u?œÝg?ýa?xp?/u?ïM-ëJ¼<?}•›ýlø?–ZB‡°{?}•›ýlø?ïûÀ}L÷?QZãìȏ?CäýlwÀ?QZãìȏ?íu?3ر?¹×	€v Ý?´S†x?¹×	€v Ý?ïš"*i?†g>hö'Œ?‰}Þñö#Ÿ?†g>hö'Œ?êƐE‹‡?°w2t°üÄ?Äå¾é½Ñæ?°w2t°üÄAGN3FGL J1305.4-4926@srÿÑÜ×@*¿?>Ú0cÀ9 ×{|xÀ;jmH÷Q¿âU©´]®÷@)ê'/—ó@j`_'5¿å²À²W¿çXÞ=¿âÆì]¶¿o¿ãõç]qËOTHERsbg@‡$Q'©"PowerLawNGC 4945?ïûfv4BZ?@²špe?Bf'ºQ?@²špe?ïË+¦Þ?ˆÏ~ï#'Ê?ztjҊ?ˆÏ~ï#'Ê?ïÌGÑЦ?w,ìL
ñÔ?yÜ7;þ?w,ìL
ñÔ?ïú°ê)?4(6hé?E?³\À€?4(6hé?ïöT9Vý'?S÷Ià5?Á?SWuÀì°?S÷Ià5?Á?îàÏÁ¸‹?²Ë ­š?¡ÿ"K?²Ë ­š?ï-GÍã¼í?–7ë‡U§Û?šWLhP?–7ë‡U§Û?塚¯ÌG?{"ñUK˜¦?…ÿÛáË^#?{"ñUK˜¦AGN3FGL J1305.5+7854@^"‡aˆ±@Cæ@;YrÀ:	!0Ò/ãÀ<¥šXÜ:¿ï¶ö˜'ö|@
Û'òã6ò@ߚ¯Ä¿à¤kTôÏ¿å€ÚUÌ¿æ+ö8+¬¿ã™{!ð{åAGNbll@Œg0U2a|PowerLawS5 1304+79?ïü2ròQ?O€'\ªo?>ln3Ϊ'?O€'\ªo?ïàZIçCŠ?|ÑsË·Î?o¥µò@ÕØ?|ÑsË·Î?ïy%Û(Q¥?Š¯7n3íÌ?ÛDžegU?Š¯7n3íÌ?ïýC|xîÌ?(µÛ=r$š?5äzRwV?(µÛ=r$š?ï¨~Ý3Tõ?•¯§}%þ>?…àH¥lRè?•¯§}%þ>?îÒâ-º«ì?µTOЇH?¢ÑÝ"sJ?µTOЇH?ívóרî?®aCS˜?´HaDrފ?®aCS˜?צּÂÁ?'߶ÌÁÍ?"žO]v­Ð?'߶ÌÁÍAGN3FGL J1305.7-6241@s	&ÿ}ú?ÁúŠ ,…ÅÀ80·omv%À:E\jd!é?㳐Núu@r¤@;¯@΂ÿú Ã?ïüÙ9™m¿âó^œm‰p¿ßÊ'Áe¤¿æÃx;%OTHERsnr@°/žƒä&PowerLawKes 17?ì¼jÎøB"?¾©ý¡Î=Ý?º©ˆ=ëb?¾©ý¡Î=Ý?îôKn	ë3?´öºU•¢ƒ? »IaLÕ?´öºU•¢ƒ?ç¢p¬ª1[?¶FunäI?릫J?¶FunäI?ïI"åÄQ?zÚÕÆ¿ñ3?–ß[£Gué?zÚÕÆ¿ñ3?æ)¦Ùx?Ì:OFº#¨?Ó¬²MùÔ?Ì:OFº#¨?é|·5-UÆ?Ê5¡og?Ê
#+J¨è?Ê5¡og?çÌ•)¿?¶ë‹á—‰?ÐgÒÕ­ú'?¶ë‹á—‰?ìÚ"¡Ñ²¡?ŸÎ¯¿º"e?¹.êòNQø?ŸÎ¯¿º"eAGN3FGL J1306.8-2146@s:É?¯Bx@Dyá`xÀ:I9¸ˆr*À;•"ô έ?Ô¸>Ã5@¨ÇÄû@@,Qy‡Ö¿æùx`}²ø¿Ü÷q¾*À¿á¿°ÁË´@¿åÌÔ^çl
AGNbcu@¤˜"`ªdÃPowerLawPKS 1304-215?ïýo6;Ù?34Ùî¡Èb?4†O¹…º?34Ùî¡Èb?ïÈsÎÑ+N?ƒ¥ZÔ4U?{Ɖ«é<?ƒ¥ZÔ4U?ïÓ_ÞxR?uD¢†O'?vPùtc?uD¢†O'?ï`¶Ñ¸ÄØ?t`}"'n?"é%ÏƜõ?t`}"'n?ïñØå´Ð,?Zƒêä
?\N5"wÇ?Zƒêä
?ì¶ÞÖåv?¾\ Èj›?ºI	HÔO?¾\ Èj›?ï•c/‹o?ˆÀÊÐÍ?Š§4Õee?ˆÀÊÐÍ?éŒv£þÖ?±ða"5)í?˙Î%p¨?±ða"5)íAGN3FGL J1307.6-4300@s!] l‡@3Ň?úÁÓÀ8yÜ>Y×ãÀ:øž0Ø ¿Ö3ãVüæñ@A×*É­3?ýf	AGH¿ÄNñTÁx¿áæF!'9¿Óôõ~"¿×´]a§\AGNbcu@¨Èm'hr°PowerLaw1RXS J130737.8-425940?ïôkÆ2åí?Q´Ê, {B?W(sh¹Ç?Q´Ê, {B?ï×ÚI."Š?zºÎ
ä?tۃ'®¬?zºÎ
ä?ï¸o¦½)Ó?
c‡?+?ä?ßue?
c‡?+?ïü¢
9,$?'ºèé³~?:ï"G×!h?'ºèé³~?ïê'¹æ?b2T¨Y>?eØáLpyð?b2T¨Y>?ï*Ï|TN?©} zˆ?š¦w%ä1?©} zˆ?ï¬ZØØbœ?‡Ö·µ£
h?"éIÔ6,ö?‡Ö·µ£
h?ï⺕ʃ?b
hzL?mEkõ?b
hzLAGN3FGL J1308.1-6707@sþÀ//˜À4›ÀzÀ8kË^7üÀ;ȯ0ړ¿çÒ:"T'@"ÿŸ‡ð@™ÿ…Vl¿ä…H=JR"¿ç_ωÿ¿æf  Øxä¿år›ÞàæAGNbcu@ˆ_>«6zPowerLawPKS 1304-668?ïþç7meÅ?#£Þÿm˘?!Œ†Õ´<9?#£Þÿm˘?ÞPi?™Y"ì—µ—?‰Ö<Hkå½?™Y"ì—µ—?ïº)p€Šn?~¶HÕõ~?u£ëŒ~?~¶HÕõ~?ïÿœÛöéß>ü`[ð·°?Éèïác>ü`[ð·°?ï÷ƒûÞÄW?Q4r¬O"¹?Pøû±®?Q4r¬O"¹?í
ÀBQ'?Žl®ÚÛ?·©ýñC4ï?Žl®ÚÛ?îàøûvOà?šT7cZE?¡ðpFã4?šT7cZE?ïûÑÍñ¸?8×CTò?@¸Ç7˜I~?8×CTòAGN3FGL J1308.7+3545@Y8¬À½ÊÑ@T'Zà f¨À9®"ƒ‡ß]À;߅¨K
E?×ôNšÜ~Š@zŠô[é@ÚD€"
¿âŸ ®1'¿ä°ýëü¿äNdíÈùa¿ì´@d|´åAGNfsrq@‹§ÅoPowerLaw5C 12.291?ïù ½1EÀ?I©¾csÜ?K}'RD=?I©¾csÜ?ïɧoßФ?®I'37£?{,GüÙÝê?®I'37£?ïfÃÁ¾ÚN?‰!lsT?"'‡Ë"R-?‰!lsT?ïõóÌèÝ?;ð§V×?ThGå6n?;ð§V×?ïùŒYÚ_?Lšý±ç$|?IΜ… ™|?Lšý±ç$|?ïM.ré¡?£ª—eŠô?–Z1¹[aî?£ª—eŠô?ïw7ÍX?•x;ûÙª¬?œ'(«?•x;ûÙª¬?ïÁíYE|È?u-KÞ<ñ)?	SmÏã?u-KÞ<ñ)AGN3FGL J1309.3+4304@[Έ~¿"À@Ri*ùš‹À8¤D¡À›À;Cä1m`V¿÷¥Ýað_ú@±«3J?þù_Js¿äBûxdsP¿Ù|ÙW¿׾íñµn¿ä ËR+úbAGNbll@™—­à
qPowerLawB3 1307+433?ïüŸ¥n±[?0i…cþ?;ӟ)ƒ?0i…cþ?ïêÿÃDË?r.ŒÏ–‰¤?e<ºÀ5³?r.ŒÏ–‰¤?ïÑgç£pf?y§Þ6ô·6?wL!é5A?y§Þ6ô·6?ïÿ©[·†?Œ|ùüd?©Ñ)}Q?Œ|ùüd?ïøz‰Í¸?J}»a̎0?O¢Ñ£‡Ô?J}»a̎0?ï}½™íÁ(?—Q·5ivð?HLÅ·vþ?—Q·5ivð?{¸>°?…?­1Tus?€™ú{Þ?…?­1Tus?ïøy&ßc?R³!™oŠ¢?Nd?c'º?R³!™oŠ¢AGN3FGL J1309.5+1154@söÍÀÓg@RŒ "µ7À9¿þÆDÀ;®ÛÇ4Ý?ߌð;Å[@¶EF0@%6€o§?î2†wÓÌ¿äp®·h•¿Ô
Û«X*¿ë®Ž
ÒÚAGNbll@œ›u%FPowerLaw4C +12.46?ïŒE.nŽ?¯ØuLˆD?Œî´rÌ ?¯ØuLˆD?ï¯ˆ:Ä?'€Tž†b?‹üÔ$Іû?'€Tž†b?íÌM)1…? ™zªN?±—¨nAÔ? ™zªN?îr|ž%g?Ž8¶®Ù?¨Ø6cö—?Ž8¶®Ù?íì̨Jó?°ó-º.Ì?°Ÿ™š½¨d?°ó-º.Ì?ì™Tx¹`p?Á.Äq?»5\:4üƒ?Á.Äq?ì.&X?©‹=I,\?¾ŽÏw]?Ý?©‹=I,\?ç¦tÕ%G?¸_{¤[×|?гUµqÅ?¸_{¤[×|AGN3FGL J1310.2-1159@sc@@IOjNÚYÀ:4Þ]	À;§£3vO?Á"Ç<6‰v@
Ãvõ׈?üÂÀ¿xPt¿èãeJ\š‹¿Ð|û3ßοæÒYÏ:w?Ѥ\&'²AGNbll@µæ©º^5?PowerLawTXS 1307-117?ïõLéù¿…?†èqAVy™?Uf+¿‰µÑ?†èqAVy™?ïÙhò?'73…é?sK¸if?'73…é?ï³áhÂ{?x÷iØZ¥`?ƒ¼&M@?x÷iØZ¥`?ïü*¿,Œa?0òÆ0ìÄl?>ªŸ£…ö?0òÆ0ìÄl?ïén\î²??cuOÊ?f'£+jÉA?cuOÊ?ï ¹¨MÅ?¥_1¤ùÛ?›èÞäh?¥_1¤ùÛ?ïDP~l?'ÏEÏ¢R?—uðG%X?'ÏEÏ¢R?ï­öZº¶ ?"¡Ë†›\?"'iG" ?"¡Ë†›\AGN3FGL J1310.6+2446@­öàF§.@UFãåîÀ:¯3‡	WÀ;à_?³UX²Â·*@
U¡¶ž@jÿ¨AR¿è´ Â>¿é)"R#J¿Ý)nÛ¢J¿é¸ÞصZ¸AGNbcu@¡÷>šPowerLawMG2 J131037+2447?ïÙ@(—¬b?š²í¯n¸²?s_ë©Úúû?š²í¯n¸²?ï·T Á?‰H"l©¹‡?x¼V
L÷"?‰H"l©¹‡?ï`{k0P?Õ‰}Ðaî?"ü0*Z?Õ‰}Ðaî?ïÇ0êÈO?gÐ,Á&?|{çkLe?gÐ,Á&?ïë¡C'r?n€¼kg?r?d^䗼Æ*?n€¼kg?r?î3zÑàæh?¾.r¢<ˆû?¬ÈRᲃ?¾.r¢<ˆû?î¬göo™§?œI®=Î>R?¥9€–r°'?œI®=Î>R?í'#8¥t*?°[Cõ*?¶Ææ:Ô^´?°[Cõ*AGN3FGL J1310.6+3222@Ugáßîè@TÓ¤à¹)À8éqHA¸À;2ªýo?ô6°x®<"@IG¨¶)@8ž_&+8¿âr<Í)®¿ã`=þúW±¿äjg="¿èºùŽ‡ÿAGNfsrq@EÃAž0LogParabolaOP 313?ï÷3ßf¾Œ?ewÞ9'ìÓ?Q˜A"ÇÆ?ewÞ9'ìÓ?ïßûmVV?ŒW4Ȟ9È?pvg'dç?ŒW4Ȟ9È?ï™%K'Ï?‡ÕYŽ;Â?‰¼v³þ"1?‡ÕYŽ;Â?ïöÍ ‡J??òi|3?SÂdÁ±æ??òi|3?ïõ´h©¼?VŒ=²à^ò?T—/îmy?VŒ=²à^ò?ï;}Þ8k=?§'	#˜µ?˜D5'üq?§'	#˜µ?îîpx/ˆü?˜;S@®kÅ?¡ø}ãW>?˜;S@®kÅ?ïê@Õ)µ?bô1v<l?eΌC(?bô1v<lAGN3FGL J1310.7+5515@]I^_0çÿ@NÓ# 8ÜÀ:V÷~0ˆÀ<
 Òrÿ¿ó&—ºo@¿ênô)ˆ@7»Ñ+¬¿èi>Tpè¿é¯"4LZC¿åjY­"¿ÖÅZ¡¥ñ[AGNfsrq@…É'RT`ªPowerLawTXS 1308+554?ïÿåØ>üJ¯Ë™×™>êæ졈é>üJ¯Ë™×™?ï씃¸ºO?h†ÍRCoÈ?ck|5g¹J?h†ÍRCoÈ?ïÊIxÍz?+?µ&ÜÆ?züÛ&ŸB?+?µ&ÜÆ?ïÿóÁ¿c¿>Í|a|Óö>Ø|J"œ8Y>Í|a|Óö?ïÿª¢«f ?Æ¿LÀÊò?WFÒ‰$?Æ¿LÀÊò?ïq"ËÏKØ?¡ô?¢?K?'͆'¦é?¡ô?¢?K?ïy¾ŽàFì?'RFæ°?È.)Œ|?'RFæ°?ïÿ$Rş²?Ñ.O}?u«g+×µ?Ñ.O}AGN3FGL J1311.0+0036@sB¡ Ï@Oˆ×ÀEÕÍÀ:¦.fDØwÀ;­À8iÓÙ?›j)?@vwY}Ë?ø¹€C‡>?î7¡Zî¿Ð
µ|Æq‹¿îw}»þ¯"?í0ÿ1#
¡AGNbll@ȱŒí'hsPowerLawRX J1311.1+0035?ïi"Qþ>N?ŸìEšRº?'Ûµ¼ÈšN?ŸìEšRº?﷔Oòum?¤Ø\-?»?'ìˆÎ¾?¤Ø\-?»?íwÏHŸ?£¬£ß5?´G‰"=	?£¬£ß5?ïéßd©ø·?e"æ"Ar?f ›a?e"æ"Ar?q襛?ªW}ñ¾?¦õ(ß½ØM?ªW}ñ¾?íµ¹ç±™Y?Ádeý?²R0ÂAµ?Ádeý?ë-gc?­-¾íû–p?ÃJcӆqÁ?­-¾íû–p?í¦™Xç?½ìGH`cd?²Ë7÷=8Æ?½ìGH`cdAGN3FGL J1311.8-3430@s;0À&Ì@<.Bßx üÀ7vßY—KÀ:þ™‰©aŽ@ŸêŸñw|@ª1ëàcX@Yèb|¿ß\-WÑù¿â`ЛŸ"l¿æ!±U¢ô·¿ì?@]EÞåPSRPSR@"FÂ&€PLExpCutoffLAT PSR J1311-3430?tÀW /GÝ?yÓçí;a"?ïÖPö›0?yÓçí;a"?µ7֕cn?ÃãŠÃ+Ó?íY-¢‹Â?ÃãŠÃ+Ó?ÉVž$÷8å?°+ý!èØÓ?éªXvÂ1Ç?°+ý!èØÓ?ˆ®ªñÝ\Ð?sjobÆí?ïETaÅÝ?sjobÆí?gbᄾbö?cóî1õé?ï蝣?cóî1õé?£Añܹšd?¸d¹ÓVò?îËàâ+
?¸d¹ÓVò?·e-ùòј?¨"î«=?íZ@Ïd=?¨"î«=?UԞG¿4p?O‹¥\Ǒ6?ïõ±9­?O‹¥\Ǒ6PSR3FGL J1312.5-2155@sVŸ¶M@DV}€^_1À8¢kË*5^À;9ÜO σ?ñlP5L"@Ž©-
z,@™#@¡Û²¿Ý©á§òš3¿ÝŸ^Ï('¿á¯ýã¿ç:ˆ»ê–%AGNbll@—žÑ·PowerLawPKS 1309-216?ïœÏ\Û3~?"ì/B×£½?ˆÌ(É3 z?"ì/B×£½?í†+×Z€?°5Û²¦ˆ?³Î¡Fâ}?°5Û²¦ˆ?ïX0ÕØ0¦?VÞW:ƒÇ?"ùåF±¹M?VÞW:ƒÇ?êAº–0?œv
"yˆ?Æù£µ§A?œv
"yˆ?î|}) ‹?ªëГÃÑ?§(8.IÞS?ªëГÃÑ?áð"m6B?Íi{¾+8,?Ü»Á%"|?Íi{¾+8,?ë)+ßp­+?±gDƒ®?Ã[P'=KT?±gDƒ®?ֈ9×´~Å?®¾Úý¯F>?ä»ã%Àž?®¾Úý¯F>MIXED3FGL J1312.7+4828@\We^(ªC@QiÿãzŽÀ7Ägˆ¥UÀ;ýG¾Ûs?ð¾Eہpƒ@ lf*"Š@Y?ñ½ß¿Þ.3>ƺ9¿ãØ:Ö.#¿áNÊwvÈο䝞ö>¤ðAGNagn@~ˆ¿±[W?LogParabolaGB 1310+487?ïÿ'þ¼Lç?
Ÿ•-fB?@OÖÑvd?
Ÿ•-fB?ïâ	÷?'»OS¬?mîñô$X¾?'»OS¬?ïÓË'?w
W×3Vd?vq^Ó?w
W×3Vd?ïÿýS}U–>¬£dœ
>µc˜À >¬£dœ
?ïÿw—(?-\J}3?R¶ÿ®?-\J}3?hf‹?–Mÿ"ˆz?Žx,ŕR?–Mÿ"ˆz?ïÏm\é~Î?L¯çQóê?xIQzÂy?L¯çQóê?ïÿþ1Á¢>¸¾ña¼Ð>¬ãú*›E>¸¾ña¼ÐAGN3FGL J1312.7+0051@s­›6†¥@Ožm?ž{À8Óî{s=åÀ;‰Oçžà*?ÿˆ¦½@°z‰^
'@öp
Y.ð¿Þ¤ÍÔJð¿Úï}XgÂ~¿ç¢o-Ô¿í9"Paí0PSRPSR@Š-ô¢3œPLExpCutoffPSR J1312+0051?3Í †L?8첍Cw?ïý†GϙÓ?8첍Cw?Áìs-§·?Î{´®jX†?ë"Ü#4–?Î{´®jX†?Ɔíž?«–_¦¤\%?ê^[Ä» ?«–_¦¤\%?¡,w@N?"þ™¶e{\?îí8Œ'Yû?"þ™¶e{\?P+ÝaÍà³?K¶tÙ?ï÷ê"´'?K¶tÙ?´dÊ9Ê|?Ç!y!¼?ísf¹h®?Ç!y!¼?ÃÖç"t°?²%C©1˜þ?ë
y7bÔ?²%C©1˜þ?dQÆ¡•?Pm‰ó?ïë®îP¼A?Pm‰óPSR3FGL J1312.7-2349@sS6@c^@Cdó=<¡À9£úoFÍÀ;gXv¹šÁ¿î6÷'`¹v@tÎ0?üÒX_g™—¿éS''Õ¿à"ú Å‡ß¿à1oóœ´?²¯'ÓÉ/AGNbcu@±Ü•%PowerLawNVSS J131248-235046?ïþ:¶	fÜ?"÷2טŠ‡?,TŸŽôf?"÷2טŠ‡?ïÝJE?ò?€j&f}Æ?qZÝOˆŸ½?€j&f}Æ?ïèzšG`ß?a_Ñg·?g…eú— š?a_Ñg·?ïÿìýÍSc>Ø'ªÕyA>ãq÷^M>Ø'ªÕyA?ïýÞüD?/~*<f{?7#†¾[?/~*<f{?ïKÁ?XŽ?§Ó'ª‡$?–‡ØÆӁ?§Ó'ª‡$?ïÒY
YÒ&?}7kô†?vÓyEX}.?}7kô†?ïþÑBcŽ?%Í¿'³?"ëÖñiè?%Í¿'³AGN3FGL J1312.8-0424@s'#ÿï9@Mé_ªŠƒÀ8ü2Q‹ãÎÀ;"ˆTÍ·®?ßý»Õ"Ù@Ø´ž­ªž@åÏ_¤*l¿âvÂé—U¿çRhÉþÅ¿ç Q¾+¿äâ!…U<AGNfsrq@ƒEÌ~($PowerLawPKS B1310-041?ïÿs××܏?°s/¨­?…Þ3g	?°s/¨­?ï݇ô;âÀ?'ÒÿŽºÝ?q<K/£?'ÒÿŽºÝ?ïØ׬±Í?h‰ôGÿé?s"*5D?h‰ôGÿé?ïÿÖDg0?]Þ¿vØ?…9"@?]Þ¿vØ?ïÿAì+[?^tqÓf¹?Â{»)r?^tqÓf¹?ï8–œ ?«ÊGÁŠ8?˜þnþ?«ÊGÁŠ8?ï¨I¿?'ûqÃr?…à-« [?'ûqÃr?ïüxŸàæ?6¾­,p/?<;	•m?6¾­,p/AGN3FGL J1314.7-4237@s7üÀz®ó@4	›€#¦ÎÀ:Edè·äÞÀ;Ø
°÷?Î=ÊïZžæ@u!àO‹"@¨_–¾s¿çš»…Û)e¿Ý‰áT2 (¿êß¹Yí¿ÙaÆ¡´AGNbcu@ª‡+PowerLawMS 13121-4221?ïùe|[›1?PoRKèc?Jjq°t¡?PoRKèc?ïͅYú$ý?‹Üe(ö/?y=Rë)?‹Üe(ö/?ï˜P3M›?¸]vͲ?‰ëøìMa+?¸]vͲ?ïáR—ôË;?V²Çq?n­gçxÕ>?V²Çq?ïËo12Ÿ\?|'[…Óç?zHg}]½ç?|'[…Óç?îrá«E?³læÅ1Ó?¨ÑåJÔ÷?³læÅ1Ó?‹á¨°?Ÿ¹|N_R"?¦&ç?QÀ
?Ÿ¹|N_R"?í×ôKýë?§h˜'*?±@]žÆÉ
?§h˜'*AGN3FGL J1314.8+2349@½Ðÿ·ZË@Tñ9èîlÀ8ß½×fƒÃÀ;ltK+w}?å±n Ø¹P@à÷Gʙí@b,?¤Ø¿Ññ¨Ys¿ß¥!¢'¹¿áÕЪä¿á§ÊlÓÆoAGNbll@™~Åm\ûPowerLawTXS 1312+240?ïí?›BÞn?sÝ¿î?bÀd	ì?sÝ¿î?ïw¾Í}Q?£íÓBFq?'&W<-×?£íÓBFq?î²# ?¡ȕIm?£ÔÝ΍þA?¡ȕIm?îˆX}x.?ŽØI\ß6Ù?§ÚwL–?ŽØI\ß6Ù?ïâê¸ð÷Ï?rAfô¡7?mGH€ª?rAfô¡7?ìÎÎӞ^a?Å!5ö˜3y?¹‰‰c
û?Å!5ö˜3y?î¯z¯¦÷?œ/Œàx¦?¥_w™EŠ?œ/Œàx¦?å­]íƏ?¿¼0ƒ'« ?Ô¥Eæ$râ?¿¼0ƒ'« AGN3FGL J1315.1-5329@s(`ÐÕ@"p'`@3À8Π°P%À;7€ KÏâ?ú¤Q›©@C¼«Âf@}KCuJ°¿áS-ë[êH¿æî¸É÷¹¿ê£Ó€‰ìí¿ïþ[2*ʄAGNbcu@'–Ov`LogParabolaPMN J1315-5334?ïW³Gb°?¨Q¢±†¥j?•	—.%õ?¨Q¢±†¥j?êúó`VÏ<?Á4š¼Yb?Ä2~¤Ã?Á4š¼Yb?ìüî)á\?¦©E¢æ8H?¸Ž°÷?¦©E¢æ8H?êx]2?¢õʜÖÉ?ÇƉû8?¢õʜÖÉ?íÁ^À»Øš?³÷
1ÿœý?±õ	úý"/?³÷
1ÿœý?ÚI²¿8Q?ϙqÐÆU?âÛ& côW?ϙqÐÆU?ì2´Pæ2¶?«"Ù™?¾j]xÎjS?«"Ù™?ܱAvAû£?»[ô™*Å?á§_Dß/?»[ô™*ÅMIXED3FGL J1315.4+1130@t?'Àa"@RYg 5)­À:'ýýûCÀ;×íÂæ™ý¿ÃªM›œÝ@+A҈M—?ÿdï`u‹¿íYo7¿áXwŒÒ½¿ßW.e3?Á?jƒ×e'AGNbcu@­°å`A‰PowerLaw1RXS J131531.9+113327?ïÄÆ1ìÐè?µ'à˜_?}œçx?µ'à˜_?ïº\âü[?®æé™TG?~(Ç@é!?®æé™TG?ïØî'ݶ÷?wëùB㈳?sˆëÿöxu?wëùB㈳?ïÿAWtlJ?	›y	Ê?Õd‹?	›y	Ê?ïýҀb]e?JÚá'ð?1kû2c¤?JÚá'ð?ï`5ÚØS>?¢n鋭j?"ùDœ^'T?¢n鋭j?ïÀ2ÌT¼?'—bæ?暣տ?'—bæ?ïö
±'gT?SÒ՞Ü:Z?Sêœîo(<?SÒ՞Ü:ZAGN3FGL J1316.0-3338@sL^`=Wy@<ñÁ'°—À8I[	T=À;6jEî÷š?ã˜ÂÁÜö@Bv2aQ)@"ül—¿à*¶Fšæm¿åuµÃ_ªy¿å
H@5¥(¿æîÅ%ñAGNfsrq@ŒˆŠqÞjPowerLawPKS 1313-333?ïþ²"°Ô?%wHòÖ¿?$ÝØ|fŠ?%wHòÖ¿?ïÔǓ/¥¾?…r֌><Q?uœ6‰ÙM?…r֌><Q?ïÕOQCa?l?Oëœî?u{Øn»f?l?Oëœî?ïþ"feü?ü…4a¿…?&¹˜±	?ü…4a¿…?ïýo=¿B?3´åÔËhÞ?4†#@ÿ?3´åÔËhÞ?ï-¯þ,b¬?­èC"7?šJARây?­èC"7?ïC
 Nÿí?']G«žD?—ž[ûGlM?']G«žD?ïûÕÄ ¶ø?6i·¥ï?@¨í	ÊÑ?6i·¥ïAGN3FGL J1317.8+3429@UÀ4 -œñ@T-€/eHÀ:7m¾I|KÀ;ñò';×?ÊLNöeÕû@›ôgÆc@«Jàxü¿å(­Q÷x¿èYV¥ÿª¿á_«ÀHì¿ïÿ¸JÅÝ+AGNfsrq@"€hۋ¬PowerLawS4 1315+34?ïÿ•¢õ
?7w>ì?
»"@›€µ?7w>ì?ïÔ&¸¦z(?R¨£ŸB?u죡Ä,3?R¨£ŸB?ï¿ìkÅî.?që»[}'¡?€åôŒ?që»[}'¡?ïDŽ¶³…Ô?bDëEù?|=¤–nâ!?bDëEù?ïÿÊ,÷ì>þòX>úðþÕ"¢s>þòX?ïá…Û:"?ªLµR†?ŸÃÏHI©?ªLµR†?ïÑ(.ÐÖz?yCÃj¹"?wkèuè—?yCÃj¹"?íòåÍ?¡ß'Ç9?°ogyEm?¡ß'Ç9AGN3FGL J1318.7-1232@s"¿Ÿ‡ð$@HãÓ %¤ÕÀ9³ '²ÌÀ;¨—¤¹¿ï'Ž>;@™íÎ à@ǹà`þH¿äkB	K‹¿ä¼0LÎ嬿æÃq¦­Ì¿áÓÞTð®eAGNbcu@®±Ä2ÊPowerLawPMN J1318-1235?ïýG\œj?3Œ¾aŒì·?5ř҈º?3Œ¾aŒì·?ï×POèdr?^$²î¨Š?tWØ*ºBû?^$²î¨Š?ïÐö™"©.?u"Á†§2a?w"³$ý\Ú?u"Á†§2a?ïÿ_º-k|?fÊ ;un?´p;Җ?fÊ ;un?ïú¿îåGå?G¿'³»ãÏ?EDÇ<Pí?G¿'³»ãÏ?ï)9Æ[€?±v½aúæ?œZØʤ,?±v½aúæ?ï€|"r‹?°"¸"R?ø ÞRùP?°"¸"R?ïòsJ®¹?Vq)ëæ~?[j˜ýÍÙ?Vq)ëæ~AGN3FGL J1319.3+1402@t¬–ÿÁß@RØû_ò®ßÀ:Նjè¬&À;ýŌf«0?ãPŒ~^ú@H§Ž¤É?ý؜žÜ¤†¿é•Øa€x‹¿Ùï38'—¿ÙDh(¢$q¿Õ¤ýä$Š×AGNbll@²EÒ-VPowerLawRX J1319.4+1405?ïý$PõÄp?/íÝƨxë?6ÝwíÎCÆ?/íÝƨxë?ïÉ?_DÚ?~œ×Áo8?{`P|ä?~œ×Áo8?ïÉ÷Ka¹j?vš¿ÞK«?{ZZ"?vš¿ÞK«?gº¾?vU°	ÂQ?&¥<?vU°	ÂQ?ï÷×Bz+ž?LÍÎ	LØ?PQzžBØ?LÍÎ	LØ?샸íÙ?À@bÄxóå?¹ïËâ8'8?À@bÄxóå?mÛÈ
?…uä#N»Y?‡dwßñ©?…uä#N»Y?ë)iÅ/c_?³¯Úm‡2ˆ?ÃZXëBr…?³¯Úm‡2ˆAGN3FGL J1319.6+7759@^CE€<ÑB@Cƒq_¾¬yÀ:2ÂfA}yÀ;äÚÔÍLO¿‰9	`üÅ
@—½Clç4?ü'_øc)¿äé»Qп×w3£E"à¿å²R^OI?²×œù9VAGNbcu@²™™Û"ÐåPowerLawNVSS J131921+775823?ïþü¥.Æ? A<G¾"¨?#Ä3(ÃQj? A<G¾"¨?ïٍéߔ?'MUŶ?s9xOæ&?'MUŶ?ïɇjíߗ?t¡GdJÞÈ?{<J¤Z?t¡GdJÞÈ?ïýBiÿE?)8‹Sý?7uëFH—?)8‹Sý?ïú=' $p?GÒOäÎ?G`èÌ/<?GÒOäÎ?ï!³ B?©U2Zœãä?œ›ÎKSŸ?©U2Zœãä?ïDïs?é?ˆPï´žÒ?Œ®Äq•ê?ˆPï´žÒ?ïÒÉò¹Î?s¬Ã"ÐCZ?v›™à°ì?s¬Ã"ÐCZAGN3FGL J1321.0+2215@vj¿ß~€9@TlŸëWÒÀ8ÆÄŸäÀ;zŠPPzl?Óô½¨RÖ"@YÌ­ÃJ@_ÄŠŠ¿ã–¤'çã¿æݳ*u…¤¿âÐ1ú+³@¿êïgMä[×AGNfsrq@‰¼äŽŠqÞPowerLawTXS 1318+225?ïþ™±u"?=të×·8Ò?&dçœmÅ?=të×·8Ò?ïØc\#u?´:([C?sÎQñµœ?´:([C?ï'ó;‡§?†Û1'ÁÝ?`BL":?†Û1'ÁÝ?ïò̓ìÜ?C¨%üž®È?[f¦«ç?C¨%üž®È?ïÿ*Øú5C? ôƒýÕs/?¤Û"54? ôƒýÕs/?ïH]|æc)?£l¦Cԟ?–ôPjÒÇ?£l¦Cԟ?ïUsÔ°h`?'^¸/!yÏ?•Q…c¼?'^¸/!yÏ?ï {'¾Šë?|OÛTí‡?‡á6	~
_?|OÛTí‡AGN3FGL J1321.7+8312@^vÖÿ´@@íÛ L¦¢À9ˆœ×;»˜À;å#ôÑΔ¿úŸ-èE¤$@¿:òð"@"ÿï¿çÿÕJF
¿å[ËÙæC¿ä-"XÐâ¿ìຍZ)AGNfsrq@'²€ñ,(PowerLawS5 1322+83?ïþ6@¦/Ì?6bƒ°›DÏ?,›ö—³""?6bƒ°›DÏ?ïÜp±÷g?‡-*?£Õ?qǧšø?‡-*?£Õ?ï™ùffný?ƒï°rë,N?‰¦_…®?ƒï°rë,N?ïÿùq½ÔÚ>È"Oéí¶>Ê8Ýî@ó>È"Oéí¶?ïþN£bVs?2[ä)"›C?+Ê}S#?2[ä)"›C?ï,ojy¤?¬á¹[w?šr²ƒL0?¬á¹[w?ï¥&³Ñ‡?ŠÐ7"Ô®?†¾öSžL?ŠÐ7"Ô®?ïÿ•Jï+`?µ¹ŽŸD?
­JÎ<?µ¹ŽŸDAGN3FGL J1322.3+0839@t_._ú;›@Qˆ¹`~TÀ9êk#d‰À;ȓ6©	y¿í0ÇA-Øç@5KÈÊà@D_ÖT`¿åªü°•3®¿ææ*cMO¿Ì-Ìnâ¿ïù_'aÁçAGNbcu@"AÆÜ]cˆPowerLawNVSS J132210+084231?ïð&÷ª`?eIîJOÌ?_Ó±»tðÎ?eIîJOÌ?ïÛôÍÇɃ?'ù_œÜØ?r™'Éê?'ù_œÜØ?ïÅ:Ëò¡?Uã›Í$?GX«©×?Uã›Í$?ïþäL£Ð2?£÷ñ0?!»7±ÄŸ?£÷ñ0?ïè";—
?r›TkO?g{Ä3X—{?r›TkO?ï[Ù*åB ?£J¤9c?""Ú¨&?£J¤9c?îB®ý?A›? ïSbä¸?«Õ.Ÿ›S? ïSbä¸?ïòÒ‡7Ü?ZMC¬´rÉ?Z[øØÓ&?ZMC¬´rÉAGN3FGL J1322.6-1619@s›§ÿyÈ@FòÖàL'À:…zþ£ßÀ;´°t§qÉ¿öÁÊóƒÅÈ@
my=¿Î@Ùö X:)¿ãØ_'.¿å‹öº±í¿ä2Äߝ׿äuø»Ï5AGNbcu@'Sl¥zxlPowerLawPMN J1322-1617?ïýšr\"Õ?1׉"åï?3,lò²Çh?1׉"åï?ïØ[ 됐?…˜Æ»ÚR?sÒoœ¯ö?…˜Æ»ÚR?{ö"ðÚ?€B5Å5?€™hb±z?€B5Å5?ïÿ|¥&7?,1hx•?kUî(²Y?,1hx•?ïù½"(I(?HdùÐÆb?I	®æuݵ?HdùÐÆb?ï1Í˳ê? Ûy±ôc¨?™Æ_}ò|½? Ûy±ôc¨?ïu^ -?‹øҏ.†¦?'\4:B'¸?‹øҏ.†¦?ïî›Kd?`$ö·pN?aææOÃ?`$ö·pNAGN3FGL J1322.8-0938@s»î²Ñ@J9JÞ™À9ò#žjºÀ;—ÿ'E7?ßÕs順â@½×Zob9@	Ÿ#•¿ç˨÷ý¿åäÁ ØMñ¿ìböuÎÊd¿æ6É5œ!½AGNfsrq@~Çâ'@¸PowerLawPKS B1319-093?ïÿÜ??Øa%Ôsn?dwèl?Øa%Ôsn?ïÜȘ?'¶Õ¥Ê'?qöþºà°?'¶Õ¥Ê'?ïÀsgx+­?vt|gNT·?ÆL8;}~?vt|gNT·?ïó:Ca˜e?AKl¯€?Y‹y°B
?AKl¯€?ïýŽÿÚ
?@OÔÊEè5?7S‰Ö­jb?@OÔÊEè5?ï8'Î×Dž?«Jkj#Ž?˜í¦#OAZ?«Jkj#Ž?è_5¬?ˆÅ÷›'|ò?QÝãÁ?ˆÅ÷›'|ò?ïŠÙ3§;2?'O8"Ñ?‰?I³ Ï"?'O8"Ñ?‰AGN3FGL J1322.9+0435@t,@FA-@PìŸÐë?À:_nÔÉñPÀ;³gþìډ?é
Ƨ™·w@
¡×ŒÄI?ûÕP~ó{¿ïÿɯ"‹E?ïúK"	¸¿Âá‡é\¿7¿áfŸ*ÀAGNbll@´±[~ÿ—PowerLawRBS 1257?ïý1#ì÷Ã?47Þ$('=?6váŸ
kà?47Þ$('=?ïqØq4n?—õˆ &?'ÄñÜÝ®J?—õˆ &?ïÉðŠÚê?y§ '7È?{»ŽÊÀ?y§ '7È?îyå‹×Üm?'	TÜ^å?¨a§B'93?'	TÜ^å?ïø"«•'ï?IP­ï´?M­RWþ
Å?IP­ï´?ìF.?¾‰ƒCcN{?½Ìwgý?¾‰ƒCcN{?ï¶}?'Cü}˜Gç?'z?Å;€®?'Cü}˜Gç?驑Z2-?·aýñ¾æß?ÉYº—§7M?·aýñ¾æßAGN3FGL J1323.0+2942@Kš¿¨!@T¦$`1˜ÿÀ9Τ…À;"Å@'H¿ßÄßv%T@.ëí¤^@)KßÒc¿á~ÚxSp7¿àQs.ZË¿å)zûÒQz¿Ù0àí¥AGNbcu@—°,"h	ÕPowerLaw4C +29.48?ïîØmiåÍ?fß;–,rg?a'''ÜcM?fß;–,rg?ïåã¹ù5‹?|—ÿæ;?jF
ć?|—ÿæ;?ïL¶FE2?2ó…8Þ?–i7>?1Â?2ó…8Þ?ïö)¾{Œz?E"l	h1‹?S¬ƒäŒÔ?E"l	h1‹?ï¯Tùwi?†€%)ZAj?"*Áºj§?†€%)ZAj?ï1ƒ_'Ú?¨QŽ–?™Ï";Åm?¨QŽ–?î5¸e®ýÑ? h*ñý%3?¬¤y£XTî? h*ñý%3?ï±°"p?™È"–&?žiÉøP?™È"–&AGN3FGL J1323.9+1405@tì¿ðEx@RºÅ_ñ_À:1Sϊí.À;Ñ#2ý?ß;¢9¦@¡Û1"x@›·1Ô?ïÿ"77y¿¿Ý^?ðt¶z¿ãA?ØTŒÂ¿Üã?AGNbll@ 
"uPowerLawRX J1323.9+1406?ïþ9ö6~?+8rëÛ­?,n Þ¦L?+8rëÛ­?ïÄJ×-'¤?'¡6Ô¤óÅ?}ڔeÇô?'¡6Ô¤óÅ?'u–Ž?Žd.yš¼?Ûf	ø'?Žd.yš¼?ï¢mýxU?p&ï>¤óð?‡d€¨Éò¯?p&ï>¤óð?ïû(*t%t?C},"?C_VVr‹?C},"?ò¼?®¦)‰Œc?¥F ҆À¼?®¦)‰Œc?ïœÄìP<?†ê²ßègÆ?ˆÎÄá«]?†ê²ßègÆ?ìÍWC³³÷?©C^÷Í¥'?¹•Eâb`G?©C^÷Í¥'AGN3FGL J1324.0-4330e@sR°€0<@2ú!€ƒHÀ7¯¦Ç…òÀ:4>ª_º{?Ó°ÙpcI@O92¦›`@94¿zSٿ僢k80¿ésr࿕¿ç4ú|»¿çRÌÒ<^'AGNRDG@"÷ó×ÛõPowerLawCen A Lobes?í›É}?¤c?ÀfˆíqTx?³!´¹g?ÀfˆíqTx?ïȈ À?'˜ªðÔÊå?{»ïá£X?'˜ªðÔÊå?çz/­lµ?¹L§2ëVÿ?ÑÛ ¥&–?¹L§2ëVÿ?ïã¯?D­¯Ío £?`\Y2Nnf?D­¯Ío £?î6¹÷a?³EÔò÷^?¬"`U֞?³EÔò÷^?îø¹˜E9N?³kG©q? tf~@ !?³kG©q?èzÎBBÅ¢?µægèòrN?ÎÆöôév?µægèòrN?ïŠÄ›"µH?{N=åè¡o?NÙBI÷?{N=åè¡oAGN3FGL J1325.4-4301@sXA?ÐÐh@3gßÿ¯x(À7oB¸âÀ:ç|8_ÂÞ?ê1M*Þ®@U8âtª@Ÿ¹<:ï¿è:ªmHпèãÊÀŒ¿åÀæøД`¿âwÄËT/`AGNRDG@~¹ÀëíúPowerLawCen A Core?ïÇá¿çÐÎ?…F¸Ý<í­?| 	Wé?…F¸Ý<í­?ì÷œ	>Ô?¾íÙ.Qn?¸C¶|ôà?¾íÙ.Qn?ëĉ¡¡GZ?«0ð(j¯?ÀíÙyzâ—?«0ð(j¯?êò'[â©Ù?ª•p¸KvÑ?Ä5¶uX?ª•p¸KvÑ?ý¬?¨Ù«æî³?¥·.|€‰F?¨Ù«æî³?àñF¦`/?Ó+О¥?ÞÏr³?¢?Ó+О¥?éÑævl?°Ù÷§"?È»¤f&O ?°Ù÷§"?Ó}ÅÀ5‡?½©óȨê‰?æAå<t?½©óȨê‰MIXED3FGL J1326.1+2931@J8ïÝëÙ@TڿԖÆÀ:²/ÍM%MÀ;ѝx]¿ô
%\ÛÎ@…"'|Ç@Ž@?`=-¿Ú˜D¦3l$¿é¿F™cá¿ç‹ø&Ì{?ÊWÍ.Ïÿ»AGNbll@¯s}¿H€PowerLawTXS 1323+298?ïÿ-­À˕?r¾ƒ¦¢z?JHòÕ;÷?r¾ƒ¦¢z?ïàÀ|(çÍ?Žˆ€:ϔ?o?ƒ¡~K%?Žˆ€:ϔ?ï´éƒ^;A?yÂO'YÊO?'ÅŸ0XI°?yÂO'YÊO?ïÿü@C>¸p	
‰>¿~š8Õ6>¸p	
‰?ïþç€q`?$»	]!EV?!‡÷t>‡?$»	]!EV?ïY]¸S)Y?¢ÄQ'¿–Ì?"ÔH÷R¢Þ?¢ÄQ'¿–Ì?îíb^nö-?—Õ;º½?¡)Ú|è5?—Õ;º½?ïÿ'a8v‹?
œ"[3Ô?gµ}ô>?
œ"[3ÔAGN3FGL J1326.6-5256@sDÊ€à@#!Kãö	À8?ŽîDì™À;}\L11?æ%í‰t¢-@•‹$‹Ðƒ@ùÀ›f"¿åȨͿäʳÎ+пä±m7ˆNæ¿è|¬uAGNbll@‹©N_oÒPowerLawPMN J1326-5256?ïýŽ¦T?4D/[n?7sŠTlêÀ?4D/[n?ï¤óµ~õ?–a/ž|?†Ã?ÈQnÜ?–a/ž|?ï¾jtú5?}."k×K?€eb´øæ?}."k×K?ïü›}ä ??""aoŸ€ø?;$KØ,?""aoŸ€ø?ïùÐsþÝõ?JÀ=Ù
§¥?H¾/Ëè7|?JÀ=Ù
§¥?îJÀÃ?¾^òԞR?¯ûSòì'M?¾^òԞR?uæÙ`?™²AT_Ýô?¥¥(£J8?™²AT_Ýô?ïõišè?Jð޼Г{?U,Êí_?Jð޼Г{AGN3FGL J1326.7-4727@sQ§€w‰¤@-÷`¿]xÀ9]5õ…R»À;ZxOœöE?ýèªMñÐ@È?ânÂ?âC`èo?ïþ¤žv¿Ðû÷\ÃOv¿å­Ðrû¿îÂh?"zNOTHERglc@™ªdÂø8LogParabolaOmega Cen?ƒ`ö¹}?—Y:ž*†?ﳑú‹Cb?—Y:ž*†?Ê)O&%?ƝEo9¸w?éºõ¬6w?ƝEo9¸w?ÃÔ7'ß"?­»½`Et?ë
òˆ>?­»½`Et?ÒʊÕRú›?²Zñ9fô™?暺•V'²?²Zñ9fô™?…mzE°?•¶Qá=ƒ?ï©Ã¾^º?•¶Qá=ƒ?±–"Ö}a?¸²ùÚ$Ï?íÍ-}Å0T?¸²ùÚ$Ï?¿õÐ;2?²6ŽT?ì_ýxš?²6ŽT?­ñÉB•!?Ÿ?p¡¡Ó?î ãkänn?Ÿ?p¡¡ÓPSR3FGL J1326.8+2211@
o}ÿ_F7@T#kà"êçÀ8¤ðÂuZöÀ;f's"L?õ-wTuM4@"Ëõak€@svënοâî›
²á¿æ¡99mÆ¿è›–ýïܿ璂/‰tLAGNfsrq@#9ÀëîLogParabolaB2 1324+22?ïùð1‰m…?P*në÷?H?:i9ªÉ?P*në÷?ïŸ‡mâ? <Ä_¥`?ˆ<ߨs[? <Ä_¥`?ï,Y'm€a?"^bÄÇ?štÍ°˜%á?"^bÄÇ?îû¤3%œG?ƒùÀc°? E¼Ññ¾Ž?ƒùÀc°?ïö-Zùm6?Uºà¼Çß¼?S¥JŽVâë?Uºà¼Çß¼?í¼¨Xèé'?Â#´Ð¸&?²½7èË?Â#´Ð¸&?îñMÝOô,?™Fª¨B{f? ë"(mK?™Fª¨B{f?ë÷Š¸Û?³=%–®?È!×Á•?³=%–®AGN3FGL J1327.9+2524@7·_}>@Th—×5ÜÀ:üײÙ܀À;úé¦Ù¿®É÷G")ï@Æç¨pL?úڒ€Ê÷¿ïÌ»N9Ö?å¹Q
ô¿êlMäF?áªÅK#>ôAGNbll@Á÷¯\(õÃPowerLawNVSS J132758+252750?ïÙP©öÅ?§w€Øª?sWô—á‡?§w€Øª?ïâ¿Cæùc?~‡Ìô' ì?m@¼*ä•K?~‡Ìô' ì?îõÞµ=Ë#?• ÓÈ!7? ¢«GfÓ?• ÓÈ!7?ïýú§P'h?/O³»?0*Åi?/O³»?ï·{þíË?…P§Ø䗡?'!C-d…?…P§Ø䗡?ïE£ì¿í}?§Ll.Uì?—K'p™Vd?§Ll.Uì?í½}¹`«´?£þáàÄÌ.?²3°Çä?£þáàÄÌ.?ïÊ!zd~?'@ª+\?zï8%ñ	M?'@ª+\AGN3FGL J1328.5-4728@sVž²gÇ@-Ø->ýkÑÀ9=E†SÀ;2îiՇ¿ò³CÛ[@T¸ëC…f?û0ßÞøH|¿ïëâ§)¥?씪¯Ê8¿Ûù)ßCê2¿"uv'EóˆAGNbcu@Ãî2Iº^PowerLaw1WGA J1328.6-4727?ïùòy'û?D<?H6'=†?D<?ïÖÒUU{?"ì…¯ïÅ?tý–Ü4z¯?"ì…¯ïÅ?ï¼ÙTšŒ?}ºY¹¡û'?€ÉªÓ…¨?}ºY¹¡û'?ïÿßÛê™^>èw¿ð>ððX¶Ÿ…>èw¿ð?ïò™KÚ¸¸?VYŒ¾µÌò?ZÍh|ð°?VYŒ¾µÌò?ï9c?¯t	šÄ£?ØÜ>sœõ?¯t	šÄ£?ï"Ѷ–‰?ŒØ×¢1Ñ[?‹'a?UÃ?ŒØ×¢1Ñ[?ïþAßüÝê?/
78‰?+â]'å%?/
78‰AGN3FGL J1328.9-5607@sBÓ@N¤©@nÔ?²ÈjÀ7`>"E]À:ÅÁ:c©?ü©}å‰N@­ègÝßÅ@sÃ²ñ¿áäŒö·Ç¿å¦ìXáÌ¿æòhElN¿ç?¨ñóš8AGNbcu@'4‰Ô•+LogParabolaPMN J1329-5608?ïú_ñ|/?JƒCƒ¬fÇ?Fƒð' ž¢?JƒCƒ¬fÇ?ï"E[ú?˜¦¶ƒL_±?‹ .±‰Éo?˜¦¶ƒL_±?ïpTÔB¸?°''½'?'ïÕlVàú?°''½'?ïêQß_M?OûE-‡ºh?e® Ìj²"?OûE-‡ºh?ïïÀ…tQ>?b-—P0Ên?`?z³Š9Š?b-—P0Ên?íjÄ­;?ÂÙݪHF?´«÷Û$p¦?ÂÙݪHF?î·üpð?žÞ÷Ü?èk?¤€8þÜæâ?žÞ÷Ü?èk?ïá±ÒÌ?dVy–g]¤?nìNø¬"¸?dVy–g]¤AGN3FGL J1330.0-3818@ss?À	oë@7ð#¶eÀ9´8ù€ŠÀ;u±ƒ›*"?äwɘÃc@
Xâe,@>Úà5à7¿éÇúÇÔ7¿é4ÀÜ©Ž¯¿ïÿ	(®Ü¿æäy<_Š]AGNfsrq@{t—CécÜPowerLawTol 1326-379?ïõ8¯Ê?aÀ¨ƒO'?Tý®¥l¦?aÀ¨ƒO'?îz±€Ð?«¦‰¤Ø?¨^"ê'×ú?«¦‰¤Ø?ï?j_UŒ?oP±"–;?œ¸·"êu?oP±"–;?ìb}´ÇÚ? x%}(yæ?¿4ìYÁ4? x%}(yæ?ïsÆùEž?—‹#¿_ÂV?'‡ ՔoÚ?—‹#¿_ÂV?ßϜh‰‰à?ÔYø—´o¼?à1Ë»;?ÔYø—´o¼?ìÈáwB›u?¨ÙS$é?¹¸ôEë$Y?¨ÙS$é?Í÷«%eÉ?ºöä€üy?è¹6¦Ž?ºöä€üyMIXED3FGL J1330.0+4437@YeÊâ°@Q·: þ¡À:V'šx¼ªÀ<¯ÑêC?Þݳ¹DHž@rѹp¤ƒ@4¬¥Q´¿áþØöPÔ¯¿Ð×ͫοá‡À[ØÌ¿ã@	ʦyHAGNbll@¡]y™™™šPowerLaw1RXS J133021.4+444117?ïÿ"dPY?aw*Œnš?³mŽ:é˜?aw*Œnš?ïÌ_¡r£X?‹›0§Ð"‹?yÐ/;¯"?‹›0§Ð"‹?ïà
"²vN?páIåÎ?oõÝc‡1¸?páIåÎ?ï^þM"s?wJ"gŸx5?"<4£ã¯?wJ"gŸx5?ïûöúƒû^?:ðþêl²?@$RzŠÿ?:ðþêl²?î¡üï¢?¹æšÂþ0·?®EîýPé?¹æšÂþ0·?ïÂÓ*Τ'?}`Nåbe;?~–j¶:bÊ?}`Nåbe;?ê=\Nàb×?³€±	7œ?Ç
ŽÄ~t¥?³€±	7œAGN3FGL J1330.1-7002@s#ý@gÏÀ²mÀ!î'À8ñ'lÀ:óyˆ'!?÷vÏtòÆ1@ã[vsN×@:~äa"ï¿ÝFž<
å¿å$oÅy‹ ¿æÎb("Ú¿å íÅYª°AGNbcu@"ƒm=…œLogParabolaPKS 1326-697?ïü=YÁ.?=D‡ìFc?>1°ä–¶?=D‡ìFc?ïŠWjÜ(?›â¡zóî?j%Z$:?›â¡zóî??rº:?€x…*(?ˆ°*0©a?€x…*(?ïüáàëE?%{×tQºZ?8÷[iÑð?%{×tQºZ?ïöÅ4/»?S·DŽµ?Ru—³Ç·t?S·DŽµ?ì(‰ŠiC?ÈL§iw#3?¾»³¬·¥ì?ÈL§iw#3?ï:)ðh2?'s&k¹1q?˜ºÝރ]·?'s&k¹1q?ïûŒˆ"â?:zB׏¹?AÍàn*4ü?:zB׏¹AGN3FGL J1330.5+3023@L­ŸàÛx@T5iÿãzŽÀ:7²€fÃÀ;Þ¬k-v¿Ü E`Ãuq@
P¨ø².@ÌÀÀz&¿é©Æ}Rf)¿åãÀ.XÙ¿â)î`›KK¿ïÿê›ê¬²OTHERcss@"a"œwškPowerLaw3C 286?ïô0|õt?`¡³´˜é?VŞÚ'?`¡³´˜é?ïßrä"¡?†k`‡eu·?pFŽ
Ãs?†k`‡eu·?î'CeÊ#?—Ùq-¼<6?§ßëÇëÑ?—Ùq-¼<6?ïÕ6«ì5&?bl±=y,?ud©úÇ%S?bl±=y,?ïî|¢	w?múD¡éøî?aƒ^%NK?múD¡éøî?îι²y6?±Æ¨SL¬?£dÚØЧ?±Æ¨SL¬?í´xÏÍ?¤L©	g÷?²_Ì?‡u?¤L©	g÷?ìÎ(£•Ï?°‰Q®ç?¹6½	?°‰Q®çAGN3FGL J1330.6+7002@]"'þKÊÚ@G\ @hÀ:Ì°G[À;êpçɨ¿ø‡ÁªÚµ@íJsk²?ý~©E¿êö5ó›²g¿Ý3"N*ý§¿Õ	'oß¿Öˤ®YMAGNbll@©MÅÖ8†PowerLawNVSS J133025+700141?ïÿV ëTo?íXâGë?;Ûvå<í?íXâGë?ïâæ>/]?€Î.Ï[Õa?mÁŽªy"?€Î.Ï[Õa?ïìN¨¿¨?[œ!ù?c±X,Zߜ?[œ!ù?ïÿï2¸˜>ÚÐpÿ¼)>àþÊÞûm>ÚÐpÿ¼)?ïþÁÂé°D? Mgë9F?#ãÍ8B'? Mgë9F?ïM4D«+?£¢jx™Å?–]YnӔ´?£¢jx™Å?ïè»õRì¦?nF§làã?gD
¦4"@?nF§làã?ïþÄ+ÇË?$' ,À?ï?#½@lž,?$' ,À?ïAGN3FGL J1330.9+5201@[>Ùb…U@Pî`/ë€À:{ÛÑLŽNÀ;ôy±œÅž?×í3¸Fán@öÅ&@ýp N¿êœ.Á¬¿ã†6TÈ%À¿ë{䖱Í?Úö'bñ;íAGNbcu@žì'¯·éPowerLaw87GB 132842.6+521750?ïûäI·¯?I?h3Í9?@oŽéŸcÜ?I?h3Í9?ïàþé2;Å?'{"ŸÞšé?oÔ£rñ?'{"ŸÞšé?ï‡áµÎ??ˆoÁ.&?Ž;Nj­8V?ˆoÁ.&?ïü*Š‡ê?8l/XÝïk?>««ZÇ¿?8l/XÝïk?ïß$ˆu"ç?vgÃööÕ'?pm»§°è|?vgÃööÕ'?ï%®[%HB?¯ÑòŸe?›J4¢6/Ä?¯ÑòŸe?î"@õq9?¢ŸcêÒ-?®w»ñ"Ói?¢ŸcêÒ-?ï¬Ú¹Ÿsx?Š:œUƒ°?"ÉQŠd²?Š:œUƒ°AGN3FGL J1331.1-1328@sØMŸS @H!ˆô'À9ÂMFðPÀ;GÔX²H½?ì,û¶š0@›3\"ë'@ý‰€qÕZ¿Ñ«óI¿áÙRûGá¿ç%RuÿDz¿îÒÁǜG…AGNbcu@—ؐbMÒòPowerLawPMN J1331-1326?ïâ¦~?¯âñí¼³.?§…0ÿAã&?¯âñí¼³.?ïªóç¡m?‡ãQ‰åv?…Cv´	?‡ãQ‰åv?ë61`±Vá?ª²«)ã
?Ã':}:¤}?ª²«)ã
?î¤súèX?'À¼ðJ#9?¥¿¿u"ƒ?'À¼ðJ#9?í°¦o¯ª?²:ÞÅ'#÷?²z̃̉Î?²:ÞÅ'#÷?í§´ö}†?¶=ûâDzr?·*ÂY•îJ?¶=ûâDzr?è5³ 8ž?²UAÀˆ©"?Ï)3φ?²UAÀˆ©"?çÁ Ääª?±&+R'i?Ð}ܾv6­?±&+R'iAGN3FGL J1331.5+1711@uÀLSâÖ@S΀+3ŠÀ9œÔY‰RÀ;ÁÂv1µ…?ç¯hZSÖ@ڍ°e@žÿµ¿è`ñEcG´¿ê<¢óŠ|¿ØY‡±J÷¿ë¶?0†IuAGNbll@zxcÜHjÓPowerLawTXS 1329+174?ï÷ðîë?MÚÈð¿Ö?PäY#¶'?MÚÈð¿Ö?ïf¡ÁþŠ?¡r¸}a4?ŸÓ+Οf¶?¡r¸}a4?ï òûywT?w.ü?›á ‹©«…?w.ü?íh0êÈO(?—¥ÖF{Âø?´¾x¨s¬>?—¥ÖF{Âø?ïôâÆfà?`=®åò¿Ñ?Wö:€ð°v?`=®åò¿Ñ?çrŸ(h˜µ?Í­k¢TB?ÑÁ¯.Η?Í­k¢TB?îQ
§"ï? H­ßDö4?ªïU‹=Y? H­ßDö4?â9ô+q¯?À4
ÍÓ é?ی©¢?À4
ÍÓ éAGN3FGL J1331.8+4718@ZDàÚ Ë@QŒÕ£5À9ê¶NÜ&À;úp¨È&?ã¸OO§×@>Âqªa@:ßßùû.¿â"Cׁm¿él®Ž6‰¿çu*ºúÎy¿èëáÁaÅÔAGNfsrq@'¦MjOPowerLawB3 1330+476?ïþÉ4Íù.?!£_ٟÄå?#l°bð±?!£_ٟÄå?ïÐöÿŸ'?†Ä$Ó?w"€fBƒK?†Ä$Ó?ïÜdàp»?n>Ža?qÍûI'œ?n>Ža?ï[Õ[f®
?sӖ
ó>?"…Tº¢È?sӖ
ó>?ïþ°,¶Ÿí?&ÅvUO*?$ý6ÞñÛ"?&ÅvUO*?î:²Šù?´ÿ\Âk~?¬T×PfþD?´ÿ\Âk~?ï«­Þ?'@­ÜÔý'?…;ԕ¹¨<?'@­ÜÔý'?éðª"˜ö?°Ö®-œI?È=U¯ùœ(?°Ö®-œIAGN3FGL J1332.0-0508@tـo&)@L!µ'm,À7rá`؇ìÀ:ìZ
7'g@b¶<g[@%8ZåS×@fà‹q¿â†ž²)ªÁ¿ç'EÍó¿ëyÎÎÙ~¿æÚÙë'AGNfsrq@€þ´}€^_LogParabolaPKS 1329-049?ïû—ÖY?I}"[ä<?A¤Mº¯Â?I}"[ä<?ï×Û¨ÕB?"ñ#|›@?t+ ržÔ?"ñ#|›@?팾·¶:9?¤ÎÎð¢?³š
Aà:·?¤ÎÎð¢?ïú=þé)¥?:¹ÏÇ,·Ø?G2ªÚ	?:¹ÏÇ,·Ø?ïí:·Ð«?h¢"0ß?bÅHÙH«?h¢"0ß?ï
4÷·Ó?´JžOÇú'?žYafW¡?´JžOÇú'?î
ˆ!Ö?¢œ)nrÖ5?®/Zí~¢?¢œ)nrÖ5?ïùiY¼¬?J§ÞÛ r¹?JYÊ"¶K?J§ÞÛ r¹AGN3FGL J1332.6-1256@sãÛ6†¥@HZ3à\÷À8bÒ°+¬À;eä`gI?ä¼èù©#Ð@Å;'þÿ@V&o¼{¿àí)†°¿çøÛPž(¿äÑ~XºE¿ãR—K$…_AGNfsrq@'P©*0PowerLawPMN J1332-1256?ïþQaœ}$?8íXf°?*éäpûï?8íXf°?ïÔÕ3<‡4?‡&M<£é?u•f{Ùn?‡&M<£é?ï²%‹C¯F?€Y¾´‹˜?ƒv@B:b?€Y¾´‹˜?ïý<|yù?8‡DPÐ?6{g²\?8‡DPÐ?ïüµ[¨-—?=s¢ÀïŽr?:U!½J Ž?=s¢ÀïŽr?ï.X{þ9h?ªæW±nÑ?š4ð~?ªæW±nÑ?îÏYC¥‹?™LKjßg?£
o®Y\L?™LKjßg?ïö\R2Ê$?I9Qo&~?SG[]ò˜?I9Qo&~AGN3FGL J1332.8+2723@Bzòà\̊@T3
ç»À9ÛO
)N®À;꽉b걿ôËvh'¸@;ˆrTÜ%@	4 ›–t¿âÓšj\¿á%$!rk'¿åªøm©?™¿ì­Hœ•¼.AGNfsrq@‹sŠû"ŠPowerLawMG2 J133305+2725?ïíÖföÑz?^'ä¦|9?b)™IÇ-(?^'ä¦|9?ïÜêÿ½ºá?
ׄ
ç?qŠ€*‹k?
ׄ
ç?îҔêÞ/Ì?'4x'ç‰?¢Ö±QAG?'4x'ç‰?ïÿäÜZ€Ì>áp¾ˆîþÙ>ë#ޖÊ,q>áp¾ˆîþÙ?ïævãGsÃ?m+¯
f2?i‰Í)ä·?m+¯
f2?ï\˜»çæó?¡»Ôò¿?"lè"…š?¡»Ôò¿?î¦Ùn×à7?™¼~]ïn?¥'iü‰?™¼~]ïn?ïþ£Î{Ï?1º60Œd{?/Åèþ8?1º60Œd{AGN3FGL J1333.7+5057@ZÉâ!ȧ¤@P7?úÁÓÀ9PaAcwŸÀ;Çñf	IUÀ"€`¯î@wڿԖÆ@øA?ep¿ãóõ@Œ¿èb+êG9®¿áïZ|ÖÉ¿è(qcDžAGNfsrq@†‹L˜_PowerLawCLASS J1333+5057?ïÿØ£xHD>ö1ÐÍ,>ó®)ހ¼Þ>ö1ÐÍ,?ïêÞ	$Ü?k¾Æ6Ì?e!÷kâ?k¾Æ6Ì?ïäΔß0ä?wGèB
\…?k1jótD‹?wGèB
\…?ïÿÿ±yN>'B¸iüSç>ƒ¾lÅw¯>>'B¸iüSç?ïÿëÇ}œR>á¥/Jpé>ä8M"ôͧ>á¥/Jpé?ï{Ã-ÍÔÆ?¡P}ä«ô?‡šFEgF?¡P}ä«ô?ïéÕso?q¬ýY=N?fä*–y*?q¬ýY=N?ïÿùdÛKì>ÓÀ¹øÞã¾>Êl`¦.>ÓÀ¹øÞã¾AGN3FGL J1335.4-2949@s£àGÓÔ@@
%`ÙRÀ:mOŽ´À;¼Þ&'d¿ßÒkLª'±@iŠ}qð³@_Õ¬˜¥?ݟVg?Õ-¿èjmÜýF'¿ÅxÀtézÇ¿åm›?rAøAGNbll@¢z¬1PowerLaw1ES 1332-295?ïÿ!­Ç~?'ˆ€®äM?ÊIû)"î?'ˆ€®äM?ïÕ*…JéD?†u²Kі‰?uj½LN?†u²Kі‰?ïåB¾Ê?dqÒ¤wå?já½zÝ?dqÒ¤wå?ïý	P¿=Ì?%l®+sÒø?7µxÍξr?%l®+sÒø?ïÿUëÄߙ?DôT(?B€ÜÊøã?DôT(?ï9HÑ)d?¦Þ'œn7?˜ÖýŒºu?¦Þ'œn7?ïæC§…Ñ¢?k)7ÀæV?i¼X:õŽ~?k)7ÀæV?ïë¦<@?[l­Úƙ?dYäy?Ë?[l­ÚƙAGN3FGL J1337.6-1257@t_¿ƒ8.@H/öÿ¦=íÀ8Ȃ•ùÀ;G2¼î¥?÷,\Tiº@l"o^Æ@À
2ˆéH¿åCvè@v¿åÍÎ{½Ty¿é>S-¿ãù;tíŠ)AGNfsrq@†] ù	kºLogParabolaPKS 1335-127?ïüÉ-IÕ?6ÉΚï[˜?9¶˜˜¥Rò?6ÉΚï[˜?î¤é¼?§š"¤_³S?¥±nìT¤?§š"¤_³S?ï—Â2ƒÐ?"¤«R¢?Š9ρ|?"¤«R¢?ìùp*Â?˜ðEy>?¿è4~¯)ñ?˜ðEy>?ïóW
fz?a°qǃo?YQÇâóûÉ?a°qǃo?äômN¦Åì?Îü%ªßg.?Ö%b²t(?Îü%ªßg.?ïF^ĺ^?'±Éï«Q°?—4'o¬*?'±Éï«Q°?Ý°eÕê$C?¹¶ÊîØ?á'Í
íß?¹¶ÊîØMIXED3FGL J1338.6-2403@sÉ}sÉ@BÈ?`h¤À9£ó=yÞÀ;¦Ñb§•?҂Ez2¡@¾]c2Y@œGÿsF¿çoP@ñx¿å6ÎDŠã7¿ê,øËG*¿çïs
q`HAGNbcu@*ԕ*™PowerLawPKS 1336-237?ïúN'CÅä?B'žf=‡ÿ?Fźð[´]?B'žf=‡ÿ?￞fü?'·‡Bv?€fs:€ù?'·‡Bv?ï¬Ë/hÎK?|É£bFLe?"Í4,«¥M?|É£bFLe?ï\ª``ö?u¥>j¾?"j³÷©B?u¥>j¾?ïé"Õä?fÌÜØ)‡?fkëòë.?fÌÜØ)‡?ìù§UÞ
?¼u%Ü]Ž|?¸2ÅY
ê1?¼u%Ü]Ž|?îêt'çƒ?˜+اʪv?¡X¶åÚºÌ?˜+اʪv?æó1À8â?´:6u7.?ÒœŽ;Ô?´:6u7.AGN3FGL J1338.9+6532@\Êοìº@InßÜt
À:"H¶R7À<$LaØb,?Ðуüàw@K–ä³s_@(·_þs¿é~+Ž›†%¿ê…ˆ·bò¿ê¼`ºAÛ¿ïû˜Ì·ušAGNfsrq@q øßzN{PowerLaw87GB 133543.8+654752?ï˜Õ,v?ÃT,˜ölÀ?žåSœÙA?ÃT,˜ölÀ?ïËæò¬Ÿ?'Y›~€vx?z†³ÿD›?'Y›~€vx?îì~¥1l?—1Ö=
Ì?¡8e¬é>?—1Ö=
Ì?ï<FµÏŽ?~sLÕÒú?œXw%ÖrK?~sLÕÒú?ïÑÝ»1™Ö?WŒØ
ۋ?w"ˆß@Ò?WŒØ
ۋ?íX᜙:?¼³ƒ)ž4?µ8÷üÓ1?¼³ƒ)ž4?îµÿÕ§€§?ž—§¹Þ?¤ ¢Y˜?ž—§¹Þ?å+'w]Ñå?·š1µÞô?Õ¨ÛD\7?·š1µÞôAGN3FGL J1339.0+1153@uWŠ?‰'Ë@QÇ€Æ^À9ž}þ2 fÀ;™5<ø®Ó¿Ø{x´û'‡@ªtb¨kÄ?ÿrKl÷¿ÑÙ¸K>~¿ç•èµó¿Ùͳ¥g
Ú¿»û¼WgdAGNbll@£Î‰…ðoiPowerLawSDSS J133859.05+115316.7?ïýhv"w?5š6ÅgD9?4¼L"b"À?5š6ÅgD9?ïÛÓ§v?ç?'ñú;—q%?r,2R('?'ñú;—q%?ïËPøYÝ0?{HGÙ¾»Ó?zWƒâߛú?{HGÙ¾»Ó?ïþ1:NtF?/{hFÆ	?,ìXÆÿ"?/{hFÆ	?ïûiÄÙ}#?C/€.‹+?BXë6с?C/€.‹+?ïQøÈJ©i?¤H+G>s?•ÀæöªÒã?¤H+G>s?ï»u‰;tî?'/5׎+?"°ÊΞ?'/5׎+?ï真'?d
ðþ
l?hc`¤'ä~?d
ðþ
lAGN3FGL J1339.8-0133@to׿¤Æ@M"dŸ¼ÉJÀ:$5a
ÜÓÀ;Ƽ楻ç?JQÝÃ@÷«yjúö@À	Às"7¿Þ£j?^ÿ¿æ(wS¯¼¿ê¥Xl~¿ïÿÒ~ù–kAGNfsrq@†n—PPowerLawPKS 1337-013?ïéàªú4?q7Ά‰ê?fVc$?q7Ά‰ê?îð> Ìÿ"?žã½êà? üïÀqê?žã½êà?îç],q?'›¬"Æ#?¡Š',\ó?'›¬"Æ#?ì7ûvzÒü?—Ò²ÛX,œ?¾@$L)h?—Ò²ÛX,œ?ï؋kûÉ?"ˆŽ+üÐ?sºJIˆà?"ˆŽ+üÐ?æFIvGò?ÍÀ:(?ÓsmÃp?ÍÀ:(?ë2Nr¡*?²ŒÂ=:ö?Ã7¢Æ5{Y?²ŒÂ=:ö?××-g±?³j¢:¡Ž?äiL'~}?³j¢:¡ŽMIXED3FGL J1340.6+4412@XÀ`#@Qz¾zÀ:'k¢ŠÀ;â;Ñgf?æ«S	@
˨/3Ÿ??þòŽ?žPŽ¿èVŽjø'™¿èè¼J&G¿ß-Ñîäh?®lª‰gAGNbll@´žˆâe,PowerLawRX J1340.4+4410?ïÿUK> W?«'¾>¤?VªHq?«'¾>¤?ïÜ´>¶?"ïÜFgmw?q¥ó
u
?"ïÜFgmw?ïç}¡°-I?W
?Eªf?h'^Ø÷¥?W
?Eªf?ïåwô-cæ?\–ê¬Íy(?jˆU‰V?\–ê¬Íy(?ïþ<¸å[±?+RZQêë?,4n1Ý#$?+RZQêë?î³5Y÷©?°ÊåÇ¢é?¤Ì¯†ðéo?°ÊåÇ¢é?ïχaU&ð?vÀ€ï«?x<O]«—Ì?vÀ€ï«?îøÌj¯ÔÍ?œñSƤà7? s9P·06?œñSƤà7AGN3FGL J1340.6-0408@tYæ?šIÃ@LF}À?`À:¨nH²÷À;®Ù1_?Õ«j¿¸¬@Œˆ;Î7[?ÿ³»@³Nw?Û#8¥fŠ¿ÒXlŽÚ´þ¿ãÔӍêí¿âˆe邩ØAGNbcu@£"Z¹õY´PowerLawNVSS J134042-041006?ïýéi)~?+x
Ѐòí?0´¶oãÑu?+x
Ѐòí?ïÁ<¸íò·?š°¾÷?a£s	$}?š°¾÷?ïÔ5‰¤®ö?rÕ¤3¾ÚÚ?uå;ºÈà?rÕ¤3¾ÚÚ?ﳚŒÑ'?gu‹l5*€?ƒz›Ñ ?gu‹l5*€?ïúÿe%s­?BÆõ›Œú?DkX™²§?BÆõ›Œú?t¦ ?­Á¶-÷c?¥X´–?­Á¶-÷c?車£*^p?ˆh&$Äë?†ßW5hd?ˆh&$Äë?í"X¡ú»?£qÕþvSt?¶í:ïÁΪ?£qÕþvStAGN3FGL J1341.0+3955@UÑ¿íÁ9@Re¢åx•À:o±,]VÀ<ØúØy?×'þøn@Ÿß…65F@Th€Z¿èôԏ}¥·¿èÓ¾šžÁ¿ÕQ8i'û¿å|i‰'ÿAGNbll@‡"øFÜ]PowerLawSDSS J134105.10+395945.4?ïÿ‰>ñ[?ë¼o#Iu?
°n²ÿ?ë¼o#Iu?ïà1f‡üí?uKH?oΙ¢ž;?uKH?ïáòé
—?jX¨'ÇÑ°?n
¿Ž8¦?jX¨'ÇÑ°?﯍Š[Ã?ikHûªÜf?"nŠ'.?ikHûªÜf?ïþ¯FîÀ¬?,%WHµ/
?%'~Ëùš?,%WHµ/
?îh³àKì?±/"ÑG€©?©tÎ"×(B?±/"ÑG€©?ï–¡r"?†ˆ¿ˆIC?ŠOW±5ÐC?†ˆ¿ˆIC?íx@xÁñ?¥Ë;|RÂã?´=ü9áz?¥Ë;|RÂãAGN3FGL J1341.5+5517@[ú?̞ª@N3·ßÕ¾
À:aLç9`À<úˆ²Â¿Ç½²"¼¶@
s		i
[@ ^š?¿ä1æ×åÛ¿ì¥/`¯‡¿Óƒ¦K6gÏ¿â«}Ww=ØAGNbll@ˆêƒn—PowerLawSBS 1339+554?ïÿŽ¢›Ã?ožFI~?zÔ}9s­?ožFI~?ïßþWß:
?…½Û×ís?pÔåž?…½Û×ís?ïÞùÅ©B?b"zŒ1Ré?pƒ.®d?b"zŒ1Ré?ïñãޝjñ?FŠ Ç&?\8BQ·?`?FŠ Ç&?ïÿI¾á?'4ÞÚ?Üu'ëc?'4ÞÚ?ï%87G?©Ê'h…•û?›Xù7çé?©Ê'h…•û?咽¦ãrð?ƒŒNÜÓ?†XVN{â?ƒŒNÜÓ?ïh^cÁ#)?ˆýR´TqL?'ô3€übé?ˆýR´TqLAGN3FGL J1341.9-2053@sèàm"@D8ڿԖÆÀ9˜c8´|À;13~²Ž?ëÊ]ð‡MM@-ÍX7úm@/òä¼®¿ã6¢Âž[Ü¿èý,Ñø¹B¿ê˜5ôâJ¿ïÿxÓ·‰AGNfsrq@zS;£D=GPowerLawPKS B1339-206?ïó[Þ3b¿?\9ßJò?YHCÇõ1y?\9ßJò?ïÍVù ž?ˆbÔx¢/?yTƒƒ55?ˆbÔx¢/?ïG™¼(Ã?ˆZQ?—ÎS}ž?ˆZQ?ïÞd¡4,?T´¸Øó?pͯ{¦:!?T´¸Øó?ïöîÆ
ª˜?W¯BÕ¿ó÷?R"t^¯û?W¯BÕ¿ó÷?ïAՄΩ?±T)'BV?Ÿ7ÅKöŽí?±T)'BV?îø™îw"?–Œ%ªÃêN? va Ð[Ø?–Œ%ªÃêN?ïOîzúû'?ˆZë .z?–0©7"·?ˆZë .zAGN3FGL J1342.7+0945@uCoÀL‹Ê@Q5ÅÑqwÀ:a±…H©½À;¿¤àõx¾?ã¤.)wâT@	L˜ Ë<)?ýë8$®¿ïý:]L•?ïàü¬äO¿ã=ô¤"Y¿Ü±z>"AGNbcu@ªê
quŽPowerLawNVSS J134240+094752?ïüàÞ%Q?8þA¿x?8ùÕ¨ÁÇ?8þA¿x?ìÁíð!ÕW?ÀjxÍNÛ?¹ð~ñUK?ÀjxÍNÛ?ï¸,|_Ìï?€"…9•?ôàÚ¦JF?€"…9•?êµU±Q5?©ì*Эé?Å*©:»+©?©ì*Эé?ïô*ö½zä?XK'¦>™G?Wª®E‡¥?XK'¦>™G?à¿i¬ïî?Ò=šÈÌ?½?ށ,§ö %?Ò=šÈÌ?½?ï{řZb*?‹'ôÆÎÌz?‡LÑDÌ?‹'ôÆÎÌz?ÏáŽT/ñÏ?º$à¬u
æ?èœjôŒ?º$à¬u
æMIXED3FGL J1343.6+5753@[xš^»w:@Lñ€@,?úÀ:ÄNÁ.3À<rãLk¿Â»ëˆÏœá@
ÁRæVáŽ@C1¿j¹‡¿ë&n"å¿ëRf¦¿­L‰×•ä¿¿à¢ø*H¨æAGNfsrq@"\¡ÊÀƒPowerLaw1RXS J134357.9+575426?ïþÄJ}¨?.ùíúœ?#¿øÆ£|º?.ùíúœ?ï܀ýt)?"n±²—Ó?q¿(jG"?"n±²—Ó?ï¯cÈñ?…x½W•?"':]K©?…x½W•?ïùã{¦Ù?5Ì¸á?Hs­&ö?5Ì¸á?ïöÊKµ'{?X™\Ï»ü?Rki.Ùô?X™\Ï»ü?ï-Úì¨?¯€ü#Å?š]d¸{	?¯€ü#Å?îÕuïµó?ž³ìጚ?¢¨¡ù£Å?ž³ìጚ?ïÕYWÒØ?p
sü"8?uSr<¹;ò?p
sü"8AGN3FGL J1344.2-1724@t?Ÿ‡ð$@EՉ?¯BxÀ8ICÝOÒÀ;+ÔÏЍL?÷åKà¤@nŠ§ŽNã?ÿqZÜg¿ÛV×R6Ú¿âÅ¢¦Þ{¡¿âЬkêp¿æ΂&é²AGNfsrq@…]Dg8~LogParabolaPMN J1344-1723?ïý·h?/ñâÀ
º?2DÁb¤Ò•?/ñâÀ
º?ïÇò ¤ƒ`?ˆϦ³íà?|¯ÌªËÃ?ˆϦ³íà?ï©ì]5æ?ª¤Uá?…"貆zƒ?ª¤Uá?ïšD"œ™B?lFŸŽµ–Ï?‰nÛIKs?lFŸŽµ–Ï?ïúÈKfcj?Cƒˆ²‰»ñ?DÞÓSðð»?Cƒˆ²‰»ñ?îÓqÌ'ê?´
Mµº¯?¢Èî"õO`?´
Mµº¯?ï{Çð€Aj?'¤2ÇK?‡ñ¯ »?'¤2ÇK?îߎ‰¬Lá?'&"™s'Å?¢fó?'&"™s'ÅAGN3FGL J1344.5-3655@s©[ߏG0@8½¿jäzÀ:'‰)ßÍ[À;¡µç­ù£¿îjÐ;þD$@
ès(ö@t{ \ÁÍ¿Ûêj3œÜç¿â,¦|+½¿ê\Yf,? ÄNE³aAGNbcu@¡¿_¤?åÉPowerLawPKS 1341-366?ïøœGHê?VÖï¸Lž§?Lõ~ýË?VÖï¸Lž§?ïԉíݜ1?'Lòz¢†?u»	.Ÿ˜?'Lòz¢†? ¬»é?'±9Ô¦»?—âùâ?'±9Ô¦»?ïÿÁJ|iÍ>óȚf eE>ÿZ¹0Žõ>óȚf eE?ïÔ"_†ß?v•]ÃD!?uý=Í|àO?v•]ÃD!?ïM³Éèä'?š£D2̞?–I†ÆS?š£D2̞?îW§N–!?¡Hæ´m)?ª…†)^Ïí?¡Hæ´m)?ï÷ÚFb®?RUà<Ë?PKr"Æ?RUà<ËAGN3FGL J1345.1-6224@sQş±á¿ÇõS`œšLÀ7À'°H1ÈÀ:1È\$Ä?óH•$êÆ@Ctà&Ç@É'?_‡¿ÙY4å
å¿çJ'QžX¿è'}Ô¿îßé	Cu¡OTHERspp@ƒ—¸Që…PowerLaw?©çsàÓh?·Wµc¨?îaˆÎ›.?·Wµc¨?ӆxj¥?Ç/JI¾ÿž?æ<ÃÊð~®?Ç/JI¾ÿž?Õ¬ª‡Al ?µŒMþ"Ó?å)ª¼_Ið?µŒMþ"Ó?á9|lpº?ªz´ˆ$ª™?ݍ'Å‹?ªz´ˆ$ª™?˜Ã"çC ³?§E`ÌwK?ï9ãXªf?§E`ÌwK?¦ZøÝ€}?²ytbÍÄ?îšPrMH?²ytbÍÄ?'Ç,ÇG?¶ñ;²É¤?ë[Ž4ûN.?¶ñ;²É¤?»=Uê?ŸÿÓ×¥eL?ìŒ^øU^#?ŸÿÓ×¥eLMIXED3FGL J1345.6+4453@WÆ"?@QL`×óÀ7\ahФÀ;|7‰?ô¼
?Ê5@ b¼bÇ@×kŠ½‰¿àš§*s=‡¿åŠÛyŸŠ¿ä¹v?¹¿çwi^WAGNfsrq@wYGÃ
0jLogParabolaB3 1343+451?ïÿ÷]³Ô?Sã_*_L?3³!?Sã_*_L?ïç~µ£ÌŠ?uo=¦"Þ©?hJCvF‹?uo=¦"Þ©?ïÉ0^í)?}…µIƒ?{gýh–¯i?}…µIƒ?ïÿæ>°6a>Ý^/C|y>éÁBj.ü">Ý^/C|y?ïþ]lRõ¬?*Sžˆ˜?*)=zW´›?*Sžˆ˜?ïs]ßüvÖ?˜Žê¾û'ÿ?'"D˜;?˜Žê¾û'ÿ?ï¶åúñ"m?†²¡)°Ó?'FS-¢Æ?†²¡)°Ó?ïÿî£ÈWÙ>éú*®ÆOƒ>á\[`'Õ>éú*®ÆOƒAGN3FGL J1345.8+0704@u# ¤<@P‰Î€+3ŠÀ9gíO#À;™x'â3?ê·«ZŒ='@øh‹Ô¡@z¥_ö_ÿڑ]ÈÞ¿ã³MŸ<"&¿ç­Dõä"`¿é†e¨Y®AGNfsrq@ˆ×ø -àPowerLawTXS 1343+073?ïïìOÛÔ?au¥\'~?`¯ò
óÉ?au¥\'~?ïÖ¸ö´°? &I–{?tò#žÂ¯²? &I–{?ï9‹7½AÑ?Ÿ€Zã?˜Î™
/æ?Ÿ€Zã?ïÖÞ窠?XRå@9=¨?tŒ(Ð?XRå@9=¨?ïת¬š?t0"˜66?t*©ÓIÒÖ?t0"˜66?ï~sèû?¯êØV'ÞÅ?Ÿ°1}ÔÖ¬?¯êØV'ÞÅ?ì¨nþ²Å\?¨mҜh­ž?º¼ˆ
iÕ ?¨mҜh­ž?ïüÖæè=?Ž}¤©>¾‡?ž`e#"ø[?Ž}¤©>¾‡AGN3FGL J1345.9-3357@sºÎ wm@;ÊÀƒoÀ9Ý7iù˜ÞÀ;°¨YOý¿å$Ú#'Cy@.¯KÝy@ºs 
Ìã¿çvE`Ô£}¿è…ù‡¿ÞLs'·K~¿æ
z'R*AGNbcu@ˆJ'¼£PowerLawNVSS J134543-335643?ïÿ/{vK"?¦S
E²?–EÆúS?¦S
E²?ïÝ™{‰?~ÏT.ßö"?qtsÅ[¤?~ÏT.ßö"?ïçÈ¢Vè«?`W'˜³gŽ?h7]s}m?`W'˜³gŽ?ïý׆0¨Œ?LºŒ"?1CÏýÂÒà?LºŒ"?ïþèî–v$?!PiL•¨?!qð	NM?!PiL•¨?ï0Ý 4±?²µ²—Öñ ?Ÿ™äbØ¡É?²µ²—Öñ ?ïÖ²íä°ª?uÃêec?t¦ˆúiÚæ?uÃêec?ïâ#K3°?dâ*)cÄ}?mÜ´©óân?dâ*)cÄ}AGN3FGL J1346.6-6027@sZýq??ûSA§vÀ8j^IarâÀ:ˆuk¼ç|¿ÖÈ,
=ïé@ƒë²k"@‹C…¶ä¿éªÊ®Ô-¿â7Bvòû‹¿âÐ=õÙá]¿å<'íØáAGNrdg@œ*ÀPowerLawCen B?ï†/ÑÌ2k?¥•{‡ÚÐ?ŽtŒóe_?¥•{‡ÚÐ?ïo_uþ¬:?®÷sï"ë^?';½?®÷sï"ë^?ìÏðLûþ‹?¨)§i›7?¹€}šEÍ%?¨)§i›7?ïýNË?K¼³:Oã?aFsÜ5•w?K¼³:Oã?ëÝ%O›?Àø+ºæ?Ã苏jÁ•?Àø+ºæ?ìOÀÁañ?Ãëû¥?½‡ùôðz?Ãëû¥?ê?|ö(ng?°¬sJW?Ç'^Fe?°¬sJW?îû¥ƒ:e4?:yRÆ.? E§Îzº?:yRÆ.AGN3FGL J1346.9-2958@sÐe`A‰7@?_ð€0<À9»éœç+ôÀ;_šÛ¸øÚ¿é'©jz¥Á@œ¨žoAV?û熿wNÁ?çKÑ Ø8¿áµ¤g¡¿ÏUsã/Bk¿Ö¨xÊ/þAGNbcu@²!µ`A‰7PowerLawNVSS J134706-295840?ïüájÇ&Î?2¾5k–_?8ô¨ßãÏü?2¾5k–_?ïί™éš?'•*4Œ´?x¨3f
÷?'•*4Œ´?ïÙ¯Påö"?lµu«ß]?s(W«AE?lµu«ß]?ïÿW,Gí¼?ç÷ý¤ß?t€+*U?ç÷ý¤ß?ïùßc
§š?Bµ»›gÁP?H't¤â?Bµ»›gÁP?ï0AYf¤?­'IÁ…•?™üWÏ«Á"?­'IÁ…•?ïÊ6ª"Ò?|AD`/ª8?zä«…
ã?|AD`/ª8?ïúâF±•9?<9®|Â?DväBG=Ð?<9®|ÂAGN3FGL J1347.6-3754@s°>€8Ÿ"@7¥`/ÁÀ9‡"ßöÀ;l³X‡€'¿ññ­w6@rš²t@ñˆŸ¡EŠ¿ä«‹3؛¿çt½ÛB[¿âû¾ŒdŸ3¿í]0©"âíAGNfsrq@‡aÙ_í¦aPowerLawPMN J1347-3750?ïùcÍɐÇ?H ,w¥É¹?JpÈv;gÎ?H ,w¥É¹?ïÐVÊgå?‰äsŽk^?wԚípÍ?‰äsŽk^?ïeé·FÜ;?†òzFÈ/g?"BÉ"š?†òzFÈ/g?ïÿæ—W>á5¿]îÑí>éî6äž°>á5¿]îÑí?ïýu‡I="?6ŒŽ8?4SÆ@6ë?6ŒŽ8?ïG`ß
^?°ÑŒ7 ÷ž?œ·âfæ4?°ÑŒ7 ÷ž?ïVÔç½,à?"	â?•%c¢•ó?"	â?ïÿ
ˆ¢¸?±.A£'?LMwª«?±.A£'AGN3FGL J1349.6-1133@tNßÒc@HhŒŸ¶MÀ8¶ÐE®À;mÖ£æ#¶?éJ½ŸCÛ@Ûç3€`
@"³Gùi¿ãÒ©p&X¯¿äQª¶2½©¿æúC‰Rà´¿êh)pMJAGNfsrq@ˆQ]öU\PowerLawPKS 1346-112?ïïȱzç?bDZËo(ÿ?`7NÙ&Z?bDZËo(ÿ?ïÚª=€¿?ƒr0X"??rªáVMêÇ?ƒr0X"??ï1åNèŠ1?'˜w¼—Mú?™ÃV)ÍñÊ?'˜w¼—Mú?ïþëºÆ?Q2Š°Ÿ?!DTŠ(K?Q2Š°Ÿ?ïì!:ړ×?h©ï@TÚÔ?cÞÅ"¬xÕ?h©ï@TÚÔ?ï&W@"ÖÍ?±$©Á/
?›5òŒL?±$©Á/
?íKw'ÿ=Û?¦Â³ÌÔ7?µ¤Co**,?¦Â³ÌÔ7?ïýb¹³•n?2î®Å?4ê3d³#?2î®ÅAGN3FGL J1350.8+3035@I²Žÿâ£Ï@S#ÏÃøÀ9
˜®¸À;Â^VY?ì÷"úXÔ¶@«[ƒc@ø¿ƒŽ¿ÛPÎWD1¿çŽ8éð7û¿ã5MTÐ'¿êðw2!ÌAGNfsrq@ƒþ:}ªOÊPowerLawB2 1348+30B?ïý»Ë%`j?,îñ…(÷?2!§|ߗ?,îñ…(÷?ïäkë>/™?"Ãðý{Þ?k"•Õg?"Ãðý{Þ?+?ø?ƒ>":텸?Œ5"z?ƒ>":텸?ïñ‹œðô?B@¼?\èÆUù×~?B@¼?ïýø_¼lò?/…ݐØ$2?0=z÷Y?/…ݐØ$2?ïSðÐb-?£ºEp(…P?•åóºLm?£ºEp(…P?îÑY*qK?˜¾þM»Y9?¢îJn4ÒJ?˜¾þM»Y9?ïйt0?qÒVÍÚf?w£F	²Wí?qÒVÍÚfAGN3FGL J1351.1+0030@tÛz WŽ\@M⟾vÉÀ9ãÔ;kçÀ;»€õ]县ÁRڅ
@'Â("¯@€Z€ª	~¿åò@òŽ}\¿Ýúê
ò©¿å6èR¿îVÁ(ŒëAGNfsrq@'_n}VlôPowerLawPKS 1348+007?ïh¢Ö¯$?§­;ä5?²ë ±?§­;ä5?ïѕžã/?'ÊQ~j´?w50tûF?'ÊQ~j´?ì1¬]@¢Ý?¨þ;hbŸD?¾rúé?¨þ;hbŸD?ïþ7½Jgœ?1+]`~ä?,",]WŒ?1+]`~ä?ïy5	vÓ?"n)ﶳe?Ù^Û¡‰¥?"n)ﶳe?ïG
""v?¤àxl¡‰•?—Mš}õB?¤àxl¡‰•?ê­]±6k?±Ö;ÝèQ?ÅJ‰;'žU?±Ö;ÝèQ?ïñÅõÃ6?T÷\£³?\t+%‰?T÷\£³AGN3FGL J1351.4+1115@u·
?‰'Ë@Q2€	¥›À9rÄÞÁÂÀ;G²'a½?ã£àU§@š0øñBù?û^ƒþý¡?ïõ9µÙ@N¿Ð÷ñ‹"¿ÛuhŒÜF迪ªºaAGNbll@¯ÕÙ‡+PowerLawRX J1351.3+1115?ï÷¸ïRç6?PÎ4,¦?PŽ!.6"Í?PÎ4,¦?ïÏ40¼¾ë?‡5œDޞ?xeç"âs?‡5œDޞ?歹Ç@àŠ?€òýגi?…ZŽ6§Š?€òýגi?ïÒJªô	þ?b/ "¡?vÚª¦GU?b/ "¡?ïÛüˆ&T¨?qgÓÁ»#?r»ÑXËê?qgÓÁ»#?îâÎÁĆ?¬¾õñÀÔ?¡Ó㷟ê?¬¾õñÀÔ?ïS'6Y6?öN^.tã?•¹=pEZ?öN^.tã?îâh€z—S?—AÆoö?¡ÙwôæîÍ?—AÆoöAGN3FGL J1351.7-2913@sæ³ S\ž@?ӆ?IÁëÀ9}ÁÕ"äÀ;Œù)L)¤?ÙÃp*"2@ôªaâs@+"¿lçà¿ã¡[òï÷¿åã'*È¿ãÆ_׈¿ìHõV±AGNbcu@Œ
Ü]cˆfPowerLawPKS 1348-289?ïøá¹Õ	˜?Ihxs½Ç?LyX±?Ihxs½Ç?ïÈÿ›o÷?'ΕþD&?{÷€08@\?'ΕþD&?bµ?'MTÀ£S?‹X{ ššÅ?'MTÀ£S?ïƚºð›"?\¡rÒ{¡?|²¢j%Ë/?\¡rÒ{¡?ïøphŒ &?N®E?N>]¯BÙ0?N®E?îä³i,?«¶~¥Ï^?¡´Éi΢P?«¶~¥Ï^?ïN¤rŽ?'ò"ú«ÿ¹?–+|š*D>?'ò"ú«ÿ¹?îΏŠØ?–ü‡÷ñî¹?®S¶ˆ?–ü‡÷ñî¹AGN3FGL J1353.1-4414@s§?Õ%@1>c_Jé2À9YÕ£5#ÎÀ;‡ýgŸKŠ?ÝÅÔGaà½@×Nìő@¿P +"¿é‰–Ü"°¿æåÜ+8‰¿ÝìäÅ<	Æ¿é3ѳ]ÝMAGNbll@')Çy¦µPowerLawPKS 1349-439?ïÕÓ´GšÉ?v*æ@s8?u%Óó‹i?v*æ@s8?îñòbÕڊ?¨ŸÏtc? àÙÔZ%_?¨ŸÏtc?ïU½é°?ØA5"+?•^è;êÇ?ØA5"+?ígøâ éQ?'Éû?´À8í®Úù?'Éû?ïIzÞ?˜ÒºÒ˜K?–Ýp
M(N?˜ÒºÒ˜K?ãëâ
ªK?юT‰¬Ã?Ø(;åÖ«j?юT‰¬Ã?íHhѝ0?¦ñ-¥
Ù%?µ¼¹yä?¦ñ-¥
Ù%?Þ"䣝?·@¹MÆ?àõ¶
ÿ®2?·@¹MÆMIXED3FGL J1353.2+1435@v0":¸c@Qº¿ÖDEÀ9ö†º À;Á¹ã»ü›¿îy­:@Öç,õW@½œÛ½€¿ã.êiž\Õ¿è%ž8uùh¿âr2¹«¿ÞЮ›UÓ¾AGNbll@ºÞžšPowerLawOP 186?ïÿ«|u?"OH¡U?:ívÿwò?"OH¡U?ïßJµÊ	?|áð¨ý˜O?pZ¥oëM?|áð¨ý˜O?ïãûœ1é ?qP	HLK½?lcí³GÑ?qP	HLK½?ïÿšf7j>û'!¢¼È?	fbÙÿJí>û'!¢¼È?ïÿŸ'Ãê?
HD'¿»ù?:Þ~Îã?
HD'¿»ù?ï1¶¥‡Ó7?¬ç9æyÈÎ?™É+UäÑ
?¬ç9æyÈÎ?ïËd–=Õµ?|ŽÔ±­œ?zM´Ç¨	Ç?|ŽÔ±­œ?ïøec?I¡Ö³}¤?Nl€;H@?I¡Ö³}¤AGN3FGL J1353.5-6640@sP @|ÇÒÀ#7À5º¢À9]ÇËÜÀ;BЉï•?¿˜à«ù@œuÁù	?þ{``½Úì?¶Ú¡Ì˜õZ¿Ó•nË©zý¿à÷†<x4¿Ý'û»¼rüAGNbll@²}ü¬1'PowerLaw1RXS J135341.1-664002?ïñ¯Uv1¾?`XAwQÐ?\¡T—ê"t?`XAwQÐ?ïƒ`+íL?™:µýZ?9§î%tõ?™:µýZ?ïĜÖK6ñ?w/à!Ԗ?}±"Ó…Oj?w/à!Ԗ?ïäÕÕÙ?NáV«¦"y?k*áë =?NáV«¦"y?ïË"2…?|öô–Oð&?~v:"ä=p?|öô–Oð&?ëdžÊ42?ÅÏ;fKŽ?Àáä×/§8?ÅÏ;fKŽ?ïuOÛ
?†aLƒä?'VäÌ\?†aLƒä?ïå¯$xä?†>/¾ã?œCJà'?†>/¾ãAGN3FGL J1354.5+3705@RišÀ
F«@RXŸá²7À:|¼A%À;üÔyixj¿±"Jn@
(oxùt@LŸ•Ü÷¿Ü$ÖN*ÛK¿áµ¸r©¿è†ñêR¿ßó(ôy-AGNbll@ª
ÀƒoPowerLawFIRST J135426.6+370654?ïúÚ4Ù?P®eMø‰|?Eˆ–?©Ò²?P®eMø‰|?ïÜ.NÇä0?"òwØÞæÆ?qèغúcõ?"òwØÞæÆ?ïOö²pÍj?‰N~mb;Ü?–)·
¼º?‰N~mb;Ü?ïϟA2Ì?cœÛ¤s?Ò?x0_Z	â?cœÛ¤s?Ò?ïuH²T@?™æzÕéV?'V麧ø?™æzÕéV?¤a@.?±òO ¹œ?¥¥¹ëý?±òO ¹œ?들ØŇ?¸Áoªëx?Á±lœéã½?¸Áoªëx?쨉"Ó?´²Ù­H?¿Ú»´éd?´²Ù­HAGN3FGL J1355.0-1044@ts<`Ÿ@HŽ¥?À	pÀ9@'
´©À;†ºö
³¸?ì³Jð"'@'È"ÙÁ@ûÿë2>¿à\ùՐã	¿åÞcK†¿éGl°ØO¿áñ±Òº;iAGNfsrq@‹¸ -àPowerLawPKS 1352-104?ïþ%HJ,Û?, >ǧì€?-«z—HÐ	?, >ǧì€?ïÑ'ÐS"ý?†ÑnˆxþÒ?wlðR‰?†ÑnˆxþÒ?ï©	å˜0õ?yEtÁÒ*?…½†Œ5RÔ?yEtÁÒ*?ïñ&랖{?A¢Ú¿5€Ý?]²("ZP?A¢Ú¿5€Ý?ïýt÷g™Ü?7&¦–Óÿ?4XC*,oA?7&¦–Óÿ?ï牫SÅ?±–Ϫ3?ŸÅne?±–Ϫ3?îžcÑ>T,?™þ`ã‡a?¦Âî®r9?™þ`ã‡a?ï¯A×:äØ?v»÷ÿAõ?"/Š&÷õ÷?v»÷ÿAõAGN3FGL J1356.3-4029@sÀüßï¿@@4¹&Ÿ¦ùÔÀ:+qøjàIÀ;®2Ì&°¿áÆ(Ûìz@Y0‹yp@{P@4M¿èî)jª¿â°´ a'¿çÿ'z9ÏQ?Ô6aË÷åªAGNbcu@¥°»/ìWPowerLawSUMSS J135625-402820?ïûóÔ"¬}??ñHùpæÏ?@0¯õeà"??ñHùpæÏ?ïÎr&8#?Š
IéLå?xÆìÖ0ˆ?Š
IéLå?ï´dӋ¥2?uøçɄ™.?'æË©?uøçɄ™.?ïÿÀȐ/Á>ô)wò i\>ÿ›¤òpQ­>ô)wò i\?ïð¼<u•ó?]zØwö'¶?^‡‡FNy¦?]zØwö'¶?ï$t-ú9B?¨Ò‹'»Û¹?›qz@¸×Í?¨Ò‹'»Û¹?ïEåèÛ(ä?'yüå&1ƒ?—CBÝ»«"?'yüå&1ƒ?ïù¤~†;?Nø^—VE¡?In|@¢?Nø^—VE¡AGN3FGL J1356.6-6428@s^-••Àð[ b 1À7ær/ÈEÀ:µ'v©V?ñ+$®¶j@U$Zþ@|'@Y·V¿äOEAÊòú¿é>'úeƒµ¿èyæ¼É/Å¿ëÇѺ66PSRPSR@'W¶y|ÄPowerLawPSR J1357-6429?ìÍ©âÎ'&?¶oöì7?¹'°çÖøÒ?¶oöì7?ۂ$»~ÏG?Ê/gƒ"A
?â>í¢@˜]?Ê/gƒ"A
?çØÄLÿÑ?°L'74% ?ÐNwfÖ^?°L'74% ?ãYÕÃZL?­+÷¢ïu?ÙLTyKgÕ?­+÷¢ïu?á»9îÒõË?Ì]jû\¾?܉Œ"Zk?Ì]jû\¾?¬½÷puš?´5`òώö?î4/0ˆø¦?´5`òώö?Ý¿?7šÃ]?»T7Bjs?á `d2žR?»T7Bjs?º³¶®ÛÓ®?¢	>³"¨?쩉*$…Š?¢	>³"¨MIXED3FGL J1357.5+0125@u?€ß×@MæÃ`<€ºÀ:p
TÙÀ;£'wŒ(˜¿ÿ;WýB
'@x_ã@#lYA:¿ézcp½­J¿ß¿üõ‰"y¿çˆ\›Cé¿Ä…âØ|ÙDAGNbll@¢–å`A‰PowerLawRX J1357.6+0128?ïüŸ¶œ½C?<‡Ëc™P²?;I(¼ê?<‡Ëc™P²?ïޟ'x?']Øìu»?p°l;¶é!?']Øìu»?郎q¯è?}YWÇ}?†Ô㉷*L?}YWÇ}?ïÿüôv£º>µ h,nŠ>¸^°Åöâ>µ h,nŠ?ïõ™eñ:?W_]Ðlä?TÍ6@*k?W_]Ðlä?ïK	Aê~?¬X
º
€Ì?–Ö
âR?¬X
º
€Ì?ï(éuf›?"½r^8½?šâߘ2d¢?"½r^8½?ïÿrD§5?3-5Ǥe?·b‡Eƒ?3-5ǤeAGN3FGL J1357.6+7643@]ƒ5Á'ì¯@CâÍÀÓgÀ9Gêz\½À<'ÇÅý?òjêD+þá@ŒgH8¨é@ßs¿jc¡¿åq8b®1¿äÍ$oËë¿á Š.öN¿ï ¯?‰AGNfsrq@…ÿëJPowerLawS5 1357+76?ïî~LÙné?k‡©Kx,l?a³2ï®á?k‡©Kx,l?ï4$uÞ²?žËØPю.?™Ûh­#Ë?žËØPю.?ý­Y.?œ@Œ‰§
?§äà"–¸&?œ@Œ‰§
?í.UJà#?ç#ÌI*}?¶U«$¨Î?ç#ÌI*}?ïèOÎä?r§C}d£þ?g°1h™<?r§C}d£þ?ê§É¯OÓ?ÃoQH¿Xè?Å`ÙBÀ³©?ÃoQH¿Xè?ì…ü=þ"C?©Næàãõ?»Ðeå?©Næàãõ?äú¬Pwß?¶±r®Õ2O?Ö
§_Aþ?¶±r®Õ2OAGN3FGL J1359.0+5544@Z  ô×®@Mr /µÐÀ9Nû'²õ‹À;ô4-n¿ð-âPíƒQ@Ïl®)±@½¢À^ÕM¿æI6¦kuU¿ä
"£`¿ëJ.‹>ô¿æ…=å):AGNfsrq@Mšu%PowerLaw87GB 135720.6+555936?ïÿhã;?L˜Ë[I? /8ìq?L˜Ë[I?ïæÞ"?z3ïÔ¸KZ?i!sN,?z3ïÔ¸KZ?ïÅÄÛÅ@Å?yÝ4RßÍ8?}')Iu?yÝ4RßÍ8?ïÿËÞÿîý>î'4{"0>ú'TÐð>î'4{"0?ïþ;©=?j?4#ÇDð?,EmÇ@ý­?4#ÇDð?ïFH`ŽW"?ª"ù'=Á?—6óó\wˆ?ª"ù'=Á?ï|$50Ü?Œ֌"¿q?{²z¬"?Œ֌"¿q?ïüG	Ü?=g×kõ@ñ?=DzJʪÕ?=g×kõ@ñAGN3FGL J1359.2+0204@u+é>ê!@N矶êÀ:Û/fÀ;"ãiÇC÷¿Áò–‰KT@
éá·?œÎ@©Ýÿ¥G¿q&ʚ˜Î¿äk8>¤šB¿âÊ˲4^ñ¿ïê…¼AGNfsrq@–¬Î!–R½PowerLawPKS 1356+022?ï:ó\X›?™ÏµÉöº¤?˜½A'P–?™ÏµÉöº¤?ïÄ~T³z?–è›5™ù?}ñÀ»‰:÷?–è›5™ù?ë镯Cé?©Ý÷—|?ÀY©Bó´\?©Ý÷—|?ﯤPE¬?lJuíû¸?":é†Úæ?lJuíû¸?îu§­67'?¬5óŸýêZ?¨¥…0)‡?¬5óŸýêZ?îwáCãjÚ?´XÑÈ)z?¨ëÂ¥9]?´XÑÈ)z?éõ¢çK(G?±f±-Ë?È)tbÓ^â?±f±-Ë?ëŽ(:—ç¤?°i;OB{?ÁÇ_ ap?°i;OB{AGN3FGL J1359.9-3746@sÙtàM/@7#Z0FðÀ9iÀJÞJ¤À;s&îR{?è–îÞ3kV@Z?A3@0rÀ;ïÅ¿å7šÆ•P4¿æ˜û;A–ñ¿Ôì·p;Ÿ¿ÞPF¼v/AGNbll@¤Ž;Í5¨PowerLawPMN J1359-3746?ïû6ErŒ ?A#ç¯ûr?C&ꜭ,?A#ç¯ûr?ï›>w‰ú??ÌVèì~s?‰0b.¯|?ÌVèì~s?ïÚ[×è×?l%šW¨]*?rÒoÛ¨…?l%šW¨]*?ï
"'«¨?yÇ֐"f?žM}/'Xó?yÇ֐"f?ïò	'½ò?UD:ۈÓT?ZßìX"?UD:ۈÓT?êù.Â,­*?Ä{ÃMzºº?ÄD÷MKZ?Ä{ÃMzºº?ÐÞ]?ŒhW4ø¸Â?Ž÷þ	øÖ?ŒhW4ø¸Â?êßDs¢d?«8³ׯÊ?ǘ'î1vp?«8³ׯÊAGN3FGL J1400.5-1437@tnݿη‰@Fßä׆À9e=?&À;Š²@YŒc?ñáÐd±ÛZ@
ZMÕ ÛØ@d§ê9?«[ž§~¿á3(N±F'¿äÒõÚ~|¿ïÿK3PSRpsr@©ŽŸj"óPowerLawPSR J1400-1438?Í,Vф'Ô?Éë÷p :?è´êKžö?Éë÷p :?Órd'ˆ?Ј|Ìëg?æFóÍþ·<?Ј|Ìëg?ä6[EÜ¿?³­·L3¿ˆ?דHÅtF?³­·L3¿ˆ?׆ÓëW°?«?nÑ!	?ä<÷–
T(?«?nÑ!	?°§0êóBF?¼®´ÞÄ?íëâæOç?¼®´ÞÄ?ºÊtS !Y?Ä£ꟸ?즱u‹ûÕ?Ä£ꟸ?̜­=mý<?·¯1äÝ{?èØÔ°¤€±?·¯1äÝ{?¤H鞁ÅC?…óA‡Q‰?î»qeüfÌ?…óA‡Q‰MIXED3FGL J1400.7-5605@sˆ€CR@ïI$À9É÷/væÀ;!€´Ê?ç/þÛgÅ6@èhÜ7xè@ù{ßto>¿ä;v€Çˆ¿èl5†Ži¿ä~ÒJ‡…¿íˆgS\…AGNbcu@ˆ¥F
¦LPowerLawPMN J1400-5605?ïë÷!µˆ?_ž3ÜÏAþ?dÞ$}ز?_ž3ÜÏAþ?ïzµŽuVÍ?Ø™%~"?©N/Xi?Ø™%~"?îùYéo4?'ç‰Ù¶~Ò? g
cüÁÂ?'ç‰Ù¶~Ò?ïŸ_QÊ"?e"Ýn
ï¥?ˆ9h!>£†?e"Ýn
ï¥?ïꨖrÙÍ?f;l§C'?eWiSlÂÙ?f;l§C'?쎮qË|ô?Áuø"ü§?»ŠŒq¤_?Áuø"ü§?îF›SiDÎ? 'éǽ?«–JËÿh? 'éǽ?íÎ"™¡Àô?˜Ëá×Ê?±Žë2_?˜Ëá×ÊAGN3FGL J1404.8+6554@[àE€<ÑB@HÇÀgnÀ:"¤?
À<3ÿn	È׿bÓ(iª5m@ªÕ"ð¸9@¿	 g¿¿å•›Jý1ø¿ÝWp3®¿àþówJS$¿åS"ÜôWAGNbll@\ÐbMÒòPowerLawNVSS J140450+655428?ïñ ?6\ð?qÿ"í-?\¿u	')?qÿ"í-?ïܕ˜5Éï?ƒ\P€,×?qµ3úhœc?ƒ\P€,×?îôѾÏ?œ]+Mbh¾? ¾Òà£s?œ]+Mbh¾?ïèñÑsû?M™àÆn‹™?gnøòÐ?M™àÆn‹™?ïö_ðLü?ÉåÂâ@?~$ÐÒ?ÉåÂâ@?îíüi¿Ù—?°ìêF×Á"?¡ 9`'Êš?°ìêF×Á"?îè@ÂךJ?"õRÃjz?¡{óÕõ÷[?"õRÃjz?îë7l0ˆg?'¨ÐV€Q?¡L‰<'—?'¨ÐV€QAGN3FGL J1404.8+0401@uuS@N¤©@NØ_¨DÀ9±ŽXó·À;šAÿŽÁ¿þöFÖ~&w@
'ZÀëÃ?ÿ¶MAQY¿åüc«ÿ€\¿à<2m»oW¿×ć^X¥Þ¿å2'#ÒºoAGNbll@¢eùÛ"ÐåPowerLawMS 1402.3+0416?ïûÙ»ÙƗ?@ej‰@^m?@™	˜A?@ej‰@^m?ïܵÂUa?'&ÉŠÿ?qû¥*ƒû?'&ÉŠÿ?ïÏóh …û?wÝÕÚÑÀý?xK¨ÝÊÅ?wÝÕÚÑÀý?ïÿäö'©>ï"ó3Ù>ë
oÑ a>ï"ó3Ù?ïë>9C?h!Õiย?dÁÆ}¸™?h!Õiย?ïIþÕø3r?®Ì…¥×ü'?–À%B±_Ç?®Ì…¥×ü'?ï¥õäâÜó?‡<(,°g?†'†ÃÙ'1?‡<(,°g?ïülÅ{Ú?AíŽéIÃþ?<™Ôœ¯â?AíŽéIÃþAGN3FGL J1406.0-2508@t9}sÉ@A[Œ@ÃÀ9¹FMÂ*²À;ƒÈ¸kù?…°ýEÂ@"Mië?þI`½¯ù¿ÃMW<¸ÿ!¿â˜šÿR䇿Æ^,h
L׿äB
s¨fAGNbcu@©EV_Ø­¬PowerLawNVSS J140609-250808?ïû…©;'ë?A<ÈXhC?Aé[ô8+f?A<ÈXhC?ïÖÙ¢ëtO?}û"‹	œÙ?t".¤bàG?}û"‹	œÙ?ïЍÂÜð?yжÙt?w¹"÷ž?yжÙt?ï韁÷!Æ?LžòÑM·?f`}ÍÄò?LžòÑM·?ïê ,Î+?kM1koÖ ?eßÓöpäá?kM1koÖ ?îëˆ
Íjy?²B±B$44?¡G$?p?²B±B$44?ià‹gõ?ƒ^'T
ä?€‡ÌÿØ×?ƒ^'T
ä?ïe/µ'áÐ?…M"°7ò‰?"Z	J|\?…M"°7ò‰AGN3FGL J1406.6+1644@É?áAy@QoÄ`Á
À:ž°²ºÒÏÀ;ÅbôÁÞ\¿Þe¼S>&½@ÁÁnSñ?ú[~ Ai?îôÕÄ¿â–û†è¿Ý	º&_˜Ê¿¡ï¢î4¯AGNbll@½sq©ûçmPowerLawRBS 1350?ïý¦ÛMÚ?1s'¤Bt‹?2É"ºoæ?1s'¤Bt‹?ïÓßÇêÿ'?ŒaºùôIÕ?v%M3?ŒaºùôIÕ?ï˜ìà_óþ?‡C>^®Ž?‰ÄÇîâ8~?‡C>^®Ž?ïþþ|Œx?'^²ŽÑ? 5NÑý?'^²ŽÑ?ïû¨ +TÔ?A%›Np?A_8Öê?A%›Np?ïñögü?´.n§æT?ž!Þ"êΆ?´.n§æT?ïQ3¬ÞM†?â‰4Ž?•ÙŠd6O6?â‰4Ž?ïóµPH0µ?\YåhíÞ?X•_hFE?\YåhíÞAGN3FGL J1407.7-4256@s×àßÞøH@1¯3+¦À9½ø¨ó©°À;˜êË»TÕ¿óDçÈüˆ§@ÖðäJ7@Éd~Û¿â}^â'kÄ¿æ0²
»¿Å%Þ®CM¿ìR€‰ŽoÖAGNbcu@ž2žšPowerLawSUMSS J140739-430231?ïÇ«óç=?xño¢Þê?|*nn§?xño¢Þê?ïÓVÊùK?†‹|2qŽ?vTšvbV½?†‹|2qŽ?îb¤Z<â_?œ%g®¾Y?©Õº_¡v?œ%g®¾Y?ïÿùö"4?=7l©w? Áäj²?=7l©w?ï(Nsê¢? )œ"Ñ#?šö.aã¯? )œ"Ñ#?ïU'ÿVëR?›¨Fµºð?•O C]Ï?›¨Fµºð?í'W<Z'?¥L¼²}Š'?±ªGÔùï?¥L¼²}Š'?ïòÞHF¸?VºÓ9 M?ZCÿÇhW?VºÓ9 MAGN3FGL J1408.8-0751@tÝ ßÞøH@I'æ@;YrÀ8|«ÆÂǐÀ;SÀ'U'z?ïM,6G@u ,°¸@	ä ¦hµ¿âºp‰ ¿ç-þQ:kr¿åÞ°Á¿äTjõ䕎AGNfsrq@…Çy¦µPowerLawPKS B1406-076?ïþË7©î?!9Ú´ory?#L…HïYà?!9Ú´ory?ïÅ@Å~5 ?'-q遂Y?}_[w¯?'-q遂Y?ïºï'Ya?y£0>\Â?Dk'k?y£0>\Â?ï{«Ka—?p—@—(‰å?Š–˜ôˆG?p—@—(‰å?ïýC×½Ž
?9xa6jÃË?5áC?ä?9xa6jÃË?î_űê70?²ŽO˜‹Ö?ª¤ã[?²ŽO˜‹Ö?ï;"»¢ò£?"5œ@©B£?˜ˆ‹¡«®?"5œ@©B£?ìæÏËëâx?£¶Ì»Û?¸É 2øÁ?£¶Ì»ÛAGN3FGL J1409.7-6132@sÝàP7P¿±9RŸô¢`À7|[TŠœÀ9±]ïŸ_¬?ð™!ï¾ê6@‡Ý­oº@ïÀ—µ>¿âÜÌG€&¿á£Ó<Ÿæ¿å°å"«s¿ë†}]#PSRPSR@¥ÞA£n.²PowerLawPSR J1410-6132?~J'0üŠ?‹ÂNì]?ïÃjûmìd?‹ÂNì]?УôÂÆIâ?È}~ï&òf?箞œÛ?È}~ï&òf?ÐA0ç¡?±æ©<Bß?çßtxçŒ0?±æ©<Bß?ß·–žO?®bˆ‹T\y?àu¤4°¿Y?®bˆ‹T\y?l®û÷vàW?r0žxîü?ïãQäÍ0?r0žxîü?¡ª–úªl?´@Oúíû?îç%VY[š?´@Oúíû?¨"©oÐr?±®Áºh?ëUÚÕ¤ã?±®Áºh?²'êJ‰?"S³Z¡ú?í¯¢¶èx¿?"S³Z¡úPSR3FGL J1410.4+2821@DÅk 	ŠÃ@R4¿û-2À:IÚÓöÀ;滵MTG¿÷ÖÞñ'@
‰%Bû?ÿ˜ nJ¿ì¦½!Å2á?±šnHæ\¿ä'ø<‰•¿ÊŠûô$!AGNbll@¤Š¥ýŠÚºPowerLawRX J1410.4+2821?ïü›ØŸO!??ÁÜsÜ?;!<¾nl)??ÁÜsÜ?ïãä^
ýD?‹bïs #?l¡Ìæô{?‹bïs #?ﰚp?i^?{ý	ÞT¤?ƒÙcߧˆ®?{ý	ÞT¤?ïÿÛ"'1>ðv7q·
>ò{È.š2>ðv7q·
?ïñW9¦?Z
¢ƒ=±?]PÅάz
?Z
¢ƒ=±?ïd&Í
(K? ¬4Ì¥"?"{&^Zö"? ¬4Ì¥"?ïKo=‹·ë?±èK׏Œ?–'G©Ê°?±èK׏Œ?ïúÂ8Ÿ-Ø?Hn
nË¿!?D÷áÜ»?Hn
nË¿!AGN3FGL J1412.0+5249@X‡, zû@N  	ö#À: H{™ÔRÀ;ûã±ëŸ÷?åϐé>?@éþ³ú™@L_ª	©¿ædÈÉ\Ï¿ëKúo¿ä¸%3ÒP«?Ɓ¡?Ö.ËAGNbcu@ŒW¢H"ÄPowerLawSBS 1410+530?ïÿP^«ö­?h±)̈́Ø?ô$½.W+?h±)̈́Ø?ïßI)rGÏ?€¸IàWCã?p[k+_8Ò?€¸IàWCã?ïÊÉXè¾4?pm}ä@4?z›S°ª?pm}ä@4?ïñw
tÿÿ?QŒÀ'VßH?]å‰râ ?QŒÀ'VßH?ïþAM ?4'F@þ±o?.føÚä´?4'F@þ±o?îÔYñ,?²F Üg¡.?¢ºo=±I?²F Üg¡.?ï4Å—έ?š=å[ˆ?™g_°uÆY?š=å[ˆ?ï^¿ÙÒÍJ?•;µB)Œ?"(Éò«?•;µB)ŒAGN3FGL J1413.2-6518@su`4óþÀ8Ô ~$ÉÀ9 ½zIrÀ:ï-؀_6?äI4Þ%‡@Ai×µ@j±€k^¿Ô®<ƒ¾æÛ¿èå*¡¿,ü¿å«ˆ†½Ò¿ã5ގ¿ùAGNsey@'‡Ø"t¼jPowerLawCircinus galaxy?ïÙTFµF?€`Im''?sUù؅Ô÷?€`Im''?ï6¾_™(?ªg(ccŒ?™(4Þ?ªg(ccŒ?î¨PÒ¼Œ?–²ê劶?¥zòצÚ?–²ê劶?ïZ⏵GÔ?qrµ1Ù?"£®	W?qrµ1Ù?íž×•—p8?´¡l°Y.?³	CR֊½?´¡l°Y.?çÓùÍó?ÉBY×6Þ?ÑÊäXd?ÉBY×6Þ?éÛìôEÈÈ?µg¬àPë³?ȐL.èÜß?µg¬àPë³?êéKåþïV?¦·Âm†é?ÄZÐhB§?¦·Âm†éAGN3FGL J1413.4-6205@s…ÿ@O¿çP®-ø6À6WQ'©"À9íi›¥"@+Hˆ"ôF@»¦9:3X?ÿôÀŒÉ¿Îà%¡¥,¿à;5Ý\'¿ãÇÇ)þ3Ö¿ìßØ/wåPSRPSR@"ÙOß;dZPLExpCutoffLAT PSR J1413-6205?'®DK¾2?)s¾:ÉYè?ïþ…ˆF¶?)s¾:ÉYè? ôėÜñ?¼"k"ýtÏ?î𳶝­È?¼"k"ýtÏ?~£Ô7ÿŽ?†æÛօ?ï¸W°ý?†æÛօ?V•|+®?E'Ê/é¾Í?ïôµwNHÁ?E'Ê/é¾Í?4-V=ø?(p|›XIç?ïýšiù?(p|›XIç?‰‰œKz§¼?¬>»d‹?ï™Ù͑?¬>»d‹?yºÌBÛì?yIïTçƒ÷?ïÌäŠ-ÀØ?yIïTçƒ÷?+ä†É54Ç?'Ő4Â?ïþA·¸ò?'Ő4ÂPSR3FGL J1415.0-1001@tæÿëJ@G׌àM³À:1¨oö2!À;¢\Gÿs?ñÇQ'ºÚ@I O–@I@ô\ mf¿æV*ۏ¢¿ê&J¿éÔ)¯É(¿á»z	äãÍAGNfsrq@Š;eÉäPowerLawPKS B1412-096?ïÆ@á$P?'P[XßsÒ?|ñ_ypWú?'P[XßsÒ?íâôV?¾©©+£>?·w27Ê?¾©©+£>?îEnãÒ<?—> h£?¨©V'A?—> h£?ë阑u¢ˆ?¡]4+´An?ÀYº)uß?¡]4+´An?ïª}P§|?‰ì¬ï•WH?…`«ÏAÀA?‰ì¬ï•WH?Û¹Áë®\?Ñ0">Þ.–?â#{Š(Ò?Ñ0">Þ.–?ìz{|R?§V´YÈÐ?¼/,'ür?§V´YÈÐ?ÖsÖL¹}?¾'¥ï	Úí?äõFÙ£A?¾'¥ï	ÚíMIXED3FGL J1415.2+4832@VÖÿÚ@S@Om€6EÀ:9¤$èîÀ<™RKý/?ÒõË'tÚ@çŠizî@Y¿Xš÷¿ìX¬Œîîé¿ã€—.5¿Þø¢æ@ޏ¿é«ÊCZ°AGNbll@€îÒáïsÁPowerLawRX J1415.5+4830?ïýªŽ?7ùø&Sß?7B­g°Åt?7ùø&Sß?ïÝã£Jj?v…[j#%D?qs<É'?v…[j#%D?ïÀ­²URB?|&ãz«pE?©&ÑçC?|&ãz«pE?ï›ä%óž?lÊójŽg?‰9ï£àq?lÊójŽg?ïöÑP¯Ü?_Ýy9[z?R]^Nm·ñ?_Ýy9[z?î†þuÖ	Ñ?±p7Åp
u?§¢Ÿbí?±p7Åp
u?îÛI{/\u?šîù"')?¢KhMæ¬?šîù"')?ìuf¿I?©þFgN‹?¼QëôÊ·?©þFgN‹AGN3FGL J1416.0+1325@) -@P}MÿÒ³—À9·Ät8·À;ÃûkEÉ8¿ä‹×<oûn@°1вŠ@èS`¥1R¿å4—Ö á¿ã2δX¿ãp	Ö©¬¿çˆ\¢d»¹AGNbcu@Œº/ìVÕÐPowerLawPKS B1413+135?ïÿ;ŠxG?&Îå#¸p?Ž³éшÁ?&Îå#¸p?ïß²QÁ¥?ƒ¥H>ª*!?p&óã}Å~?ƒ¥H>ª*!?ï¡4ªÎí†?Œ´"J9?‡²Õ]rªu?Œ´"J9?ïþµÝÇñÇ?ôÈ\Y·?$¢ oÖs?ôÈ\Y·?ïÿR%fÁÖ?9Ü`ŽÄ'?»J±Jõœ?9Ü`ŽÄ'?ïWd~Àám?¥ÉF0ý(?•p0zØJ?¥ÉF0ý(?ïxV|I¸Â?ŽR¢7˜Šµ?õ0oé¯Í?ŽR¢7˜Šµ?ïï²ÕLDŸ?Y§´¾{äÇ?`M*½á'?Y§´¾{äÇAGN3FGL J1416.1-2417@th€àe0@AT"¤%À9éé8=^/À;ŠçɨU?ÁJdI£@
ÕQßñ—²?ý¤ã!"ž¿æ´ëQ+Ÿ¿Ôàña׋m¿Ñ¾Ò¬=hʿܱѪAGNbll@®¼©ã½PowerLawNVSS J141612-241812?ïýt¤0/?04&«kû:?4ZàNÉa"?04&«kû:?ïÕw¨½4?'ô™¾,Hý?uD~"}ñ?'ô™¾,Hý?ïÝ/œ‹ø'?nr¡š[kÐ?qh1´"^Ð?nr¡š[kÐ?ïç¦tso?Nêáû Q"?håYc±Ô?Nêáû Q"?ïø•³¹‰?J"n‹ð"?M©0q¢Pæ?J"n‹ð"?ï«<î?¥õußìii?Ÿ*Ÿp0/?¥õußìii?ïÖ`q¯Å«?wÀS€?tÏÇ'm>‰?wÀS€?ï3YèÃg7?‰ªo–®?™"ÂÞü%?‰ªo–®AGN3FGL J1417.8+2540@@Âõ`iÍ#@Q§š_ý–™À:@җçè²À;äOªb>¹¿Â>­"@$f@wBIP«ê@O=f'@¿ä=ÆҌÕ;¿ç#HÖ¢Rj¿ÐèyïÊŒ¿Ør%åumÉAGNbll@›×:)ÇzPowerLaw1E 1415.6+2557?ïÿv ~?‡f¯-Ž?<ŸtöìŠ?‡f¯-Ž?ïáKÍz?ƒ°É%î:?n´à·XM÷?ƒ°É%î:?ïèaß=3?`_JÑ}B?gž "âTØ?`_JÑ}B?ïú,xÙÛ?1š+ÁnQê?EËM2ó#L?1š+ÁnQê?ïþìǾðì?'Ð7ï8h?!3'-AÏ?'Ð7ï8h?ï%i&ä¬?«÷ñ%¸Ž?›RÝuüx?«÷ñ%¸Ž?ïÒ?Ð¥tn?xä 'M?và"ˆ™?xä 'M?ïΰMÿÖÿ?rÆjà¯?x§Øê'?rÆjà¯AGN3FGL J1418.4-0233@uYO d#–@JÓ`IôÀ8C¾vÈ´9À:§dd-§?óșSù|X@¿¿
œ?òº0»3È/¿«1œÜ]þ¿ÓٖG2L6¿É|µ»ÁÀ¿Úñ3ÉÜžAGNbll@¡,5?|îLogParabolaNVSS J141826-023336?ïæÅzŠ­?~<ìÊåD?i:ú'Óêà?~<ìÊåD?ïœ6ôL²O?¤lÒëcªŽ?ˆòBßüP?¤lÒëcªŽ?ì¤ö®akš?¨î&îê?ºØJŒô£3?¨î&îê?ï,i{!g?{K'4'
?šrЖ«´–?{K'4'
?ïõK{Jñb?a8¥Gå¬?Ui	%ûË?a8¥Gå¬?íëÎjU?»JIUÎ-?°¡½dßZ?»JIUÎ-?î|ü˜Ÿý? "þ
m¨`?¨06tH`É? "þ
m¨`?í‰w·`mÃ?cÈДü?³´BDŽžk?cÈДüAGN3FGL J1418.5+3543@O˜XóÖ&@Qe`&±EÀ8Ml+¢E:À;<º¾­OY?ê6©a…"Œ@<cϳ1@w§€)Ú¿á7ñÓdÞ¿áQ<{0wí¿Ý&¤ãu¿åh^©AGNBCU@"éûçl‹PowerLawNVSS J141828+354250?ïÿy]ö¤?4ÓWÍn?ÔGÈ«ç?4ÓWÍn?ïçüHety?}GÍ5à²?h·m0¯F?}GÍ5à²?ïÑÙ°Ls?'ð{h?w'ú˜Ö‡?'ð{h?ïÿdz)Úç>ëó*É}>ü&m´TA
>ëó*É}?ïÿbP¾E? ãÌ1®[e?S®–¦
Å? ãÌ1®[e?ïd@À?ž0ð±ÛA?"}\öEÚ?ž0ð±ÛA?ïÇï%oÙµ?'Œè耗H?|mie/?'Œè耗H?ïÿ¾A¢?c?
"äô-?oˆª¶zœ?
"äô-AGN3FGL J1418.6-6058@s•òä?À« ƒ¥‰À5ä°S'ˆÀ9m˜‰Ï@>Î 3ý@¶ÓŠ"Õ?þäE,ã¿ÉrÔÚs«¿â"èCî
Ý¿æl@·øvÁ¿ì·ã8ÉöPSRPSR@¡\@IQƒPLExpCutoffLAT PSR J1418-6058?UÕH·Ê?Z»Ô¸ñ§?ïõ[ºn"?Z»Ô¸ñ§? ^zÔosú?¼Q²i
#™?îúRÍq?¼Q²i
#™?'ã1_•ß?–?ÚWò&Æ?ïpæuH	7?–?ÚWò&Æ?vÇxÍå²<?dӀšÖ?ïÒq`?dӀšÖ?C&ÙÞ2?>væ?ïû6môO?>væ?†Sô/v?¥ƒÕ>Äã?ï§þ°/ïB?¥ƒÕ>Äã?"ÙŸÄ~?'xAû»X?﬙ƒŸ1^?'xAû»X?T"vØ0¦?Q•²Pž?ïõ½Äœ&½?Q•²PžPSR3FGL J1418.9+7731@]@ù?ò^W@CK. &{•À9óË!ÑáàÀ;àƏ›éÖ?êªÑI´)@'œH 'Â?þ€*Ÿæºµ¿èr|Ë$#¿ÖH
y©ÿ¿Û¼^ØÏ¿à¼#p·<AGNbcu@¦¼¿b¶®}PowerLaw1RXS J141901.8+773229?ïû:#oúB?cÄÓ~¡¬r?CrÙx¼S?cÄÓ~¡¬r?ïÇc­_°P?‰?å{ÍßO?|N)mÛ?‰?å{ÍßO?ï‰õŠ?'ج¬¬Rý?~»{—T2Æ?'ج¬¬Rý?ïmÇqvÃ^?pÐï¾3ÂÓ?'GØÌ)?pÐï¾3ÂÓ?ïù¥¸-Oç?Fš.i¯^ ?IiŽ¼,m?Fš.i¯^ ?íðI½ýëÂ?¶/ÎÓ õ?°}²~•l?¶/ÎÓ õ?ïI-ùëò`?——&#Š†?–Ú@»¢|?——&#Š†?ì¤Ð
ÁV?£Î{‡?ºÙ'õO<?£Î{‡AGN3FGL J1419.1-5156@sÆ>KZ@!?" ÔÇÀ99rãLkÀ;¦-?Û¸çV96@
úßڛ—@LÀL
ð¿æKQýE2¿éH<Mtc:¿íù•©
³?¹Éi–AGNbcu@'Wq!«KsPowerLawPMN J1419-5155?ïÌH#ôë"?ƒÓ,¹L·q?yÛî?ƒÓ,¹L·q?ï•fªGÖ?"%tÄþR?Š½&_¼ÞU?"%tÄþR?î¾~Š
yT?–ß!€[ĝ?¤`Q½?–ß!€[ĝ?ïÓ5¯ß?gÐD;œJè?vvå6ël}?gÐD;œJè?íU³‰Àï°?´žMme?µRc±Š?´žMme?êmTƒÝ<(?È>¦Ά¥?ÆJ­ð‹`?È>¦Ά¥?ë¿ÅŸ©K?²Žköůý?ýéZÖ?²Žköůý?ë÷–!j?¹øœÎEE?À!§zWßæ?¹øœÎEEAGN3FGL J1419.5-0836@u
–Óõ¶@H0%ŸÌ¹'À9ñ|¯~À;~i%]‡›?ópò~$@BwsÔä@)ñŸj¿ÕÐÉöG‰E¿äZÚŒ_¨¿ç4L—wV¿çd^¾/AGNbcu@Ž­´mÅÖ9PowerLawNVSS J141922-083830?ïý1±¨Ùþ?:™}@?6rqx![n?:™}@?ïÄù¨¼»÷?'šéSTá?}ƒ+½ÎÐ.?'šéSTá?ï0D×܆?ÄMýWçÅ?™÷e	–˜
?ÄMýWçÅ?ïrUF"?hB°éì</?ˆ£jËjç?hB°éì</?ïúa?µøu?MáhÛ?F{}T{Å?MáhÛ? ¿m?³V)#Ý!P?¥µð 
=?³V)#Ý!P?îM¦,‹4?ža ð*=ú?«%7L·-?ža ð*=ú?îEˆ<úÝ+?—q/Û{?«§|3ÁÉE?—q/Û{AGN3FGL J1419.5+0449@uâê@M®Q¿æ4}À:•ža÷À;¾Љð?Ïêé˜_ˆ@
&Î 4?ümá]?ìÅt¾:Z;¿ÔÂ
@ºt¿ä;ÝâÚç?ÔÁš	.ÏAGNbll@µÂ±&éxÕPowerLawSDSS J141927.49+044513.7?ïþS³cø¬?*Ü©œJp"?*ÄÌîÏ?*Ü©œJp"?ïÔ¡ç`?'OD™‰•?uÀuÏX£ö?'OD™‰•?ïµË粞?0]îÛ-û?'ABT‹?0]îÛ-û?ïû}ïfw%?6Uº^|?BAjæd§?6Uº^|?ïú«Êɒ[?Cú‰°=Û?EPÕYÎjÝ?Cú‰°=Û?ï:†öB«»?×ܛ-	Ò?˜¯!9bVŸ?×ܛ-	Ò?ï•ÿ
­N?…Ø¡O*Ä?Š€?Ãsä}?…Ø¡O*Ä?ïÄßàr='?€0ŒÙ¥tÚ?}ØK"?€0ŒÙ¥tÚAGN3FGL J1419.8+3819@QlT_Ó¥.@Q³çüÔÀ9˜ov°`…À;ãžs.?ÚÊ4Sf%ñ@
qœ÷GÍ@êÃyíؿݺÈÆáY¿æHÓ¿–i ¿èÀ…tQ¿ãäVpœlªAGNfsrq@ˆË>À//˜PowerLawB3 1417+385?ïñW'¯?m^NSšé?]÷RÖØc?m^NSšé?ï›Ê8eà?š¹£äÆö?‰
qôP?š¹£äÆö?ï`Ì7óÙ£?Š†óÊsža?"æy
ч?Š†óÊsža?î=d½ú£?'uó=?¬)´2»ØÍ?'uó=?î›ËÿâÇ?°%»ü²ýö?¦C?ÿK.?°%»ü²ýö?êÙàDŠá?ÇóœÍß$?Ę~í×ð~?ÇóœÍß$?ëi"Þ!?·©†RB'?ÂY쇟"{?·©†RB'?݄1þ?X?Â!VOJž'?á=çp€àT?Â!VOJž'MIXED3FGL J1419.9+5425@X"'`4P@M"ßµ§íÀ9*X R…ßÀ;Õ»¢ç¿À¹u³q˜/@©¤aÒ#@u¼ '+"¿ä%bf_¿å -êÉâã¿áC×ͪ¿äÉâb=ëQAGNbll@Œⶮ}VPowerLawOQ 530?ïÿÑÎáœ_>ò>E®­>÷}ly™R>ò>E®­?ïâ{Rå2Ó?ƒœôùØ¨?m"­Jç´ù?ƒœôùØ¨?ïéÒ÷´,?q§¼•p?f-9õñ?q§¼•p?ïûXÝ«†?.F	@ä?BœˆÌÝ8?.F	@ä?ïÿ·ÛÆ?º^
þÔÒ?	HvÑÈÉ?º^
þÔÒ?ïd'ØÚC¥?¤÷¢0¾z)?"o¤ß!_?¤÷¢0¾z)?ïÚB+Òy?|sÉ+Oµ…?rÞê0]ße?|sÉ+Oµ…?ïՑ­o—ñ?m?—·Œ?u7)(—Ÿ¬?m?—·ŒAGN3FGL J1420.0-6048@s˜jŽ:Á?Ìb'KÀ6Œd¤ÅFÇÀ9-#'Õ?öèË°íô@& ß²C@õž_§'¿äø²Ñ‡¿á—~ôt(¿åV+8p'¿ê[õ¡âéPSRPSR@¶By‡+PLExpCutoffPSR J1420-6048?Ž#DùeNg?"c#³/å?ï‡rëãq?"c#³/å?Ðlsš›;?Å²à‡¿§u?çÉÆ2²bq?Å²à‡¿§u?Ñ¢Œ4´Æ#?³WH…7´c?ç.¹å¥œî?³WH…7´c?ßw_¡¿ó?°ˆ"äaÜ?àuÄP/ ?°ˆ"äaÜ?i‹®‡d?sX¤qçáj?ïæâtÿ±Q?sX¤qçáj?¤Lϕúï?³@YŠ«'4?î»3_!?³@YŠ«'4?·ç"*b¯A?ª9ØÎ>»?íºŠnÈ?ª9ØÎ>»?¼Ô†Þ¼ñ?¤Uƒà·Ê¹?ìeo$>èb?¤Uƒà·Ê¹PSR3FGL J1421.0-1122@tõEߨq¤@Fäq_¾¬yÀ:ï!‹kÀ;¨ñ՚Ѩ?â¥hF‡Æ*@*¦ò—@ƒ{À?˝?ïðHöF¡X¿àKz'°§†¿Ü"ŒM¿é—ðJ'"ÞAGNbcu@¡4£n/PowerLawPMN J1420-1118?ïòßS•±á?_"ÏâÉ?ZAX b.?_"ÏâÉ?ïÃgmnå³?Šøc©rª—?~LI>>Rl?Šøc©rª—?ï'—cM?–G»j¸Å?œýµªœK?–G»j¸Å?ïžÜGÐõ?mZƒÝ$S?ˆHîFÊ2Ì?mZƒÝ$S?ïÞ®¸©n?s‹•Nγ?p¨£‹¬I?s‹•Nγ?î—Ü?³¾ $¢F?¦'<£~?³¾ $¢F?íÜÐpÎÒ¿?¤4¦+‰a?±|wc¨‹?¤4¦+‰a?î-¯Ã°!?—•?­&õ1Hñ?—•AGN3FGL J1422.4+3227@JÅ`Iô@QeæÀ:s¬ ›%À;ÿÀƒé.,¿Ù8Uj'Ï@­¼Åd#@zIŸÜ(à¿ê,‹5¦ú¿áØ:å6ُ¿äoÙ1^¿ïý¤µÎÐÕAGNfsrq@…\-PowerLawOQ 334?ïÒ#—pÜ?yçç'H*Ï?vî4AÎF?yçç'H*Ï?ïåŦ+½?w»fõ?j:Yê@sã?w»fõ?î¶Qó_*)?'UÞýӊ>?¤šàÌ¡f?'UÞýӊ>?ïìwáÒ².?P̬¦?cˆRÒi?P̬¦?ïÂLùOY?€x&WWª·?~ÿٙUÓN?€x&WWª·?ï <!³ç?©kÒ6ô&ç?›ø{Ätù!?©kÒ6ô&ç?í†ð'Ç?¤•âdjŒ?³ÈUã›Í?¤•âdjŒ?î¯ï¼z?›ÞåTãD#?¥>¬w¾?›ÞåTãD#AGN3FGL J1422.4-6137@s˜^`=Wy¿ä¶ŸÇ±À7¿—02ͳÀ:c""aSØ@ðfôUÒÅ@BŒ:áRk?ñ¦õºgš?ïùÎدs?¸žàLÓºŸ¿Ûæøݽ¿ëk$GSšPSRPSR@§H:û~'PLExpCutoffLAT PSR J1422-6138?X]hÁ†c?fkk
3'?ïóÑKÀ%}?fkk
3'?¢duJ"Þw?¾]ï}"h?îÙ¸«W²?¾]ï}"h?´¬Ç–'ƒI?¦Ï䛙¦?íjg
;Ž?¦Ï䛙¦? ÎX‰¡,u?‰$'1Ja?îówX.É?‰$'1Ja?SN…ó—5j?Q¸Aw?7?ïöX½9?Q¸Aw?7?ÞªC*º"?¬!rà d?WÑ÷?¬!rà d?¹/Y¼N-?¨ù8¹Ð‰?ìÚÈRÙ[?¨ù8¹Ð‰?''œ—?v×`ÍÀÕ­?ïµ÷»¸ÓF?v×`ÍÀÕ­PSR3FGL J1422.8-7828@s9(€QÉ÷À0p‡ÀSAÆÀ:VD& }¹À;µü‹×97?ï@"§;@"Õxíҁ@\t_£S­?Í$Ø5¥m&¿ÙÆñ§³Ê¿à\2ce¼¿è)'KãòóAGNfsrq@£­¸ºÇËPowerLawPKS 1418-782?ïð˜6ù?b˜r=7U›?^ÎáÝÿœÒ?b˜r=7U›?ïSF׈p/?¥>GÒ;F‰?•—%©È?¥>GÒ;F‰?€Áäð?†[‰°ÆÆs?ˆ˜Ù՗ù?†[‰°ÆÆs?îDZ¿wœ?™z%½)C?£"äõÚø?™z%½)C?ïÎŒƼ+?‡a{þ¥£B?xž¹¯ßº9?‡a{þ¥£B?éÎ"ÿß|?ÆîoWëh?Èǝ¬'?ÆîoWëh?íÚaËՉ'?§ßq‡"(?±,ñ å¿í?§ßq‡"(?ê¿ÿ'zt?¥Aä¸è¢?Ŷ/ ?¥Aä¸è¢AGN3FGL J1422.8+5801@Ys´á¼©@K˜Z?çvœÀ:‡ëÚ¯
ŸÀ<!µ±þm?鵡,éu®@
V;Í5¨X@$û_\[ö¿ì¾§:õ|ø¿ì^êв¤F?â/ãu/×ß¿Õg¥<AGNbll@§íµÂ\)PowerLaw1ES 1421+582?ïüǎŸj"?bvåcîN?9Êá›c?bvåcîN?ïÒ0Âü¥"?"ҏYl?vçža`âS?"ҏYl?ï¯é=?†dqƒ˜)?"ºòŠA§?†dqƒ˜)?ïÌ'×(ª?m¾+A?yìêjà?m¾+A?ïú(ö¡å÷?PϺ²'ãÔ?G\&IPc?PϺ²'ãÔ?î?Ÿ.GÕÆ?¸7¢/â"*?¬
Ÿ?¸7¢/â"*?ïhÝùšá?'"E÷œ^d?'îD=]â?'"E÷œ^d?ï‰.'Q»M?ã+Ý@Â?´[«',§?ã+Ý@ÂAGN3FGL J1424.3+0434@uø›@-¹@M1πsÝÀ:…Óé÷€À;Ê(X
Þ¿Øñû	öùÇ@½Ta$X@㽀~•‡¿Ý÷›ä…È¿çñsÛDî¿åh†0ÂQ¿á¼e¦ÍߜAGNbll@èù#¢œxPowerLawTXS 1421+048?ïÿ.¼V?g½XÁð?(xÖM_,?g½XÁð?ïٍóH6¦?€lM´%z?s9bÃå5?€lM´%z?ï¦÷7{äŸ?|€¸®…?†B2' 7?|€¸®…?ï÷ð9cxö?9æ±F~Õv?P©zä'?9æ±F~Õv?ïûÈ0c}±?Foœ6ò"Ë?@ß=°…¡â?Foœ6ò"Ë?ï#-£ô‰?ª?éì@¦%?žšFZî?ª?éì@¦%?î/û	9ÿ? -þ¦TÓ?¦-Q$.	? -þ¦TÓ?ïQ
çM›?Žù¼Ÿ!&?•Þ®H=¶Ž?Žù¼Ÿ!&AGN3FGL J1424.6-6807@swp€0<ÀEÔÀH^À8l›
²áÀ;/*Ê®å?ð>¢ýñ]@{L‹Hóå@I½ 1xÉ¿ã1=¦9÷.¿ç-³;£'Œ¿çÈoè<·8¿ê™¼å¬ :AGNbcu@KüPHPowerLawPKS 1420-679?ïéfç?›¬m)û±O?f™çÀ>¯?›¬m)û±O?ï@µZrñ?¨/Ëîƒë?·é]H§Ü?¨/Ëîƒë?ï`ŽBøF?‡Q4(=?"î7¹Q[B?‡Q4(=?îò;DµÍ¾?zÀ& àœ? ÜK¸À?zÀ& àœ?ïéù;üÁ˜?k7ŒÚQ™H?fÄ0™?u?k7ŒÚQ™H?èž-û:ôH?ŅøZ¢Ái?͇H.á?ŅøZ¢Ái?îZÆ,Y?ŸQx{cd?ªSŸþ!Sn?ŸQx{cd?ê$Ðy! ƒ?©Ç&¡
	?Çl¾{}ò?©Ç&¡
	AGN3FGL J1424.9+3615@O¼ÿëJ@Qâ (zÀ9]Ô´øš±À;¦V6mzWÀ48éU™@UòŠ÷jZ@ÄÓ_ãëL¿×Gž?È¿å›ÖDg/†¿áaÍm-8¿ÕŒ8ôΖAGNbll@™ˆþߤ?æPowerLawFBQS J142455.5+361536?ïþ®5 âè? G'îÚÛ-?%ª'š%X? G'îÚÛ-?ïæÿô'¿?'ÕÍ?¤ß?iÖ/q'?'ÕÍ?¤ß?ïÛ;uª"¬?q]'A]…Ô?rbE-}Yý?q]'A]…Ô?ïÿÿÿv¡>&ÌôF~¼ >Õ#Ææ9>&ÌôF~¼ ?ïýù6|È?.%Ô`Ҙ?06M3ëøš?.%Ô`Ҙ?ïk ñqa? Ê3æ"?'›ü:ò›ô? Ê3æ"?ï¢9|^±w?…'bB€³?‡q ëÃ> ?…'bB€³?ïÿÿ˝Å>˜š"ÞãY>x¹qãñ3Ç>˜š"ÞãYAGN3FGL J1426.2+3402@LÀŸ¡ñW@Q ß@wÏÀ:R¸S™HÀ;áðT'QÌ?ãÅ-žÉ¯6@
SÛ&Éï?þÞ%ÀÕ?Ù¯L+§¤¿ß Ëkg›ß¿ÓeØÍ¿æ2¹˜½|AGNbll@¥#ZŸ¾vÉPowerLawRGB J1426+340?ï¦O‡ÿ?·Y?¼	"Y?†l?뾯?·Y?¼	"Y?ï›sî;¡?™Fá96?‰# {¹?™Fá96?ïœF¿Þ/?‰^ù/T?ˆîzÂJ4?‰^ù/T?îº8»?‡E²…±Ù?¤\w ;Û?‡E²…±Ù?ïÛÅk(Ý?zS( €ê?r9=…¿?zS( €ê?íLË3Þ?½ 6B?µŸa¥¼†'?½ 6B?îßç•Œ³?å¶‰±ž?¢Ž…ËMÊ?å¶‰±ž?éIa*g\±?µ™ôøkàD?ÊÚ{Vb>?µ™ôøkàDAGN3FGL J1427.0+2347@=}z °P@QúÿåþÍÀ6¡H2ž¸½À:ÁÅìß?é×Pô0¶N@d¬Iõl~?ûŸD®'û¿ÖÝÕL'î¿Üãȗ3ó¿Ú#¹m¬<¿Õ¼aÛ(AGNBLL@‹+JLogParabolaPKS 1424+240?ï5uv_éÜ?°‰ÝâÎæ?™QQ2Jö‹?°‰ÝâÎæ?ïàÍ°ÕþØ?ƒPp ʈù?o2O
d¿ì?ƒPp ʈù?íÏKî²÷?¦†Æ­HÚ?±… îOG?¦†Æ­HÚ?ïöíŸÈ]?=ð"wªT?R%
f…ô?=ð"wªT?ï¹_+Mzv?†RŒÒ§Ph?¨5!J¬?†RŒÒ§Ph?ï6zGï­Í?¨Ö¹	Ì]?™0¶þšªZ?¨Ö¹	Ì]?îênwA\? ׶4ÚÓ?¡Y'oŸ7? ׶4ÚÓ?ïæy+e˜?dRô£9XL?i†Ô':7Í?dRô£9XLAGN3FGL J1427.6-3305@tRÕàqÅ?@9—3 ¾¼iÀ8'ÖJúÐÀ;[Êò×ùQ¿ÔÚÍÀV‹—@»66ó²@XØ\œ8¿äB2øOÝc¿æ[k2þÚç¿æÍõbµ#¿á|RAAGNbll@…€èÍJ¡PowerLawPKS B1424-328?ïþÊlº]?0‰=h»Ø?#Y4êt
w?0‰=h»Ø?ïÇÞ݀q?'ý•ãÎ	?|ù–;©?'ý•ãÎ	?ïÎË϶ñ?t¹pÊEq?xšŒCa?t¹pÊEq?ïÿÁ,kÔö>ï´ëÐ?Ô¹>ÿiÙÈ>'>ï´ëÐ?Ô¹?ïýýã+o+?4ëß-o7?0èÄÈÇ?4ëß-o7?ï%Ìêm¶V?©ZPŸÓæ	?›Fbµ¸ÑF?©ZPŸÓæ	?ïzw®R?ŽÝ<ßîãY?±
9ïÙÐ?ŽÝ<ßîãY?ïþ6Ã¥J—?'7ÅP;?,"Ä.è??'7ÅP;AGN3FGL J1427.8-3215@tYªK@:W– hUTÀ:apÑ#s£À;±,±8ò¿Ë¯iU•D@¯~瑟$@I¾×ü?ïGΠ·p¿à^–%›Åï¿âž:Ãu`)¿×X
1/¼ AGNbcu@«X=Ùb·PowerLawNVSS J142750-321515?ïýeK^M=?>¿I@$–?4Õ£ÐíJ–?>¿I@$–?ïÌ?Œn?û
¦5Ú?y÷@}ÆlÈ?û
¦5Ú?ïÄó߂©`?|"`îo|?}†%>4b?|"`îo|?ïôôhi˜A?Cdé²qúy?V/ŒŒ?Cdé²qúy?ï÷~"ä×?P¯óž­à?QÖ hqU?P¯óž­à?îêS7îÏ?°ö$(ª?¡Z̈¼ú?°ö$(ª?ïŽE¿
,Ê?‰:Fؘ\?Œn@$i^?‰:Fؘ\?ï{H¿Gº:?…f8?ÍÐw?–èPêÁ?…f8?ÍÐwAGN3FGL J1427.9-4206@t6m
J@1Cƒ`r0ŸÀ6p`w	LÀ:€®n<ô}?þx"¹7Ē@ ·…gÞa@⾛ܔì¿ßRØȌ¿ãÙù·w·-¿ä±¤0Ëпç«)>gĵAGNFSRQ@yülAÝ"LogParabolaPKS B1424-418?ïð',ãÙ?`"8Óræ¢?^ݦ
)]?`"8Óræ¢?ï»&­Ïí¥?šïþiÍ°?6T‡Õ?šïþiÍ°?ìc üyãœ?ª1DÉó$?¼æø0ã"?ª1DÉó$?ïþëÓx7Ÿ?0ؔÈûº?!BÇô/'Í?0ؔÈûº?ïÂ:¾~¸?|Îê+}íL?~â ¬Yûú?|Îê+}íL?î¬~#؈~?½%Sn"š?¥8À¿ª#?½%Sn"š?í­F{Ùô?¥=‰^Qß?²•Ë³<ã?¥=‰^Qß?ïÿLÿb \?aåˆî¸Õ?`Õ¡æ?aåˆî¸ÕAGN3FGL J1428.5+4240@S^<Ö_@P93À9KÏf@×À;>vƒêÛ¬À0‹áu%@W]ª*5‰?ù1¶@™MC?Ðm=ú¦=±¿ÐúMƒÁk¿á
a<…í?ÐLW
l¯AGNbll@·J‹àÞ҉PowerLawH 1426+428?ïý+ª}Â?.ß¡ýò¦?7&£a}K@?.ß¡ýò¦?ïç(RÚmt?|càÑnΑ?h×­vÃç?|càÑnΑ?ïžíà™?†Ýçeû£?ˆD¾ýª…è?†Ýçeû£?ïÿÿû+§>G¬#Zôè>CgšÇµ>G¬#Zôè?ïúrÙ«f?A~Wœ
°?F4™³:º¿?A~Wœ
°?ïj;	bÌ ?1GJÂF?'¸žÎý?1GJÂF?ïL¦'¤­Ÿ?'³H['\Õ?–k-Çú°)?'³H['\Õ?ïÿÿPqvT>£Ì،|kÒ>•öíì1ó8>£Ì،|kÒAGN3FGL J1429.8-5910@s´à&Eå?õ ¿ÉÙþÀ7(g  ‰xÀ:zõ‹1÷Ê@wÿb÷*@ßaÏÓ½@†Ûw_ˆ¿Ñû@VÿŽ¿ãoÙU¶Ì¿èP]<•e¿ï	‡Q²>PSRPSR@‰NÚQÎPLExpCutoffLAT PSR J1429-5911?7¥à4åÞb?;~—ù2,?ïýD	w×?;~—ù2,?™ñ üëG?³´/Š8&?ï7øvÁæ?³´/Š8&?•@®UoF€?'T'€vá?ïUúFÇ\?'T'€vá?^­\jGE1?K¥}OÑlv?ïð©Qâ9µ?K¥}OÑlv??©ˆø¡Z?iRˆéÁÖ?ïü
ΡIw?iRˆéÁÖ?}öBn–_? 7/
¬}?ïÄõD)? 7/
¬}?{Â4Çu´?s؏Ø3‹?ïÉÔ{S½?s؏Ø3‹?,Êo«Nè?%Ÿuΰ{â?ïþ3Y<u?%Ÿuΰ{âPSR3FGL J1434.1+4203@RÄøä@P^ÀW¦À:4ûŠOzÀ<'~Ê
{¿Ù–Zê%@m÷êï]@"í¨'Ú¿äÐX؉C‹¿ã%8~‡×¿æÖ&'¼¿çF£¦@y AGNfsrq@‹²}¿H€PowerLawB3 1432+422?ïÿ®ÝTA?¬¸àµÍ?HÎf}J??¬¸àµÍ?ïß»i–v?'$PäÕE?p"K|Ÿ?'$PäÕE?ïØOSi"r?qVR•Î±È?sØV0¡Ó?qVR•Î±È?ïüL{Ðþ,?)PQu-¹ó?=œ ÿ^ê?)PQu-¹ó?ïýš7NJç?7ÂwÏfzs?3.DÀøy?7ÂwÏfzs?ïCw^}±?¤0oC
¿í?—ž1W³Ô?¤0oC
¿í?ïe#‹¨ó²?'Ìc¨õ?"[Ž‰)»¹?'Ìc¨õ?ïÉ_Ð<±?sKfˆÝ£!?{Pއ??sKfˆÝ£!AGN3FGL J1434.6+6640@[a¿7¸Ô@G±K¹ëÀ:µ´ZæÀ;õãåî¿ð(¿1-Êi@
Rß3›Ž?øCú€º$ª?Ð¥zbò"†¿À»iÝ=â¿ÓIáùR¿Ç7Tºc±AGNbcu@Ä##S÷ÎÙPowerLaw1RXS J143442.0+664031?ïýØR¼æP?4öí2àœ?1=kôä+‹?4öí2àœ?ïßÀïÁ:ë?"\9¼è?pˆ+6˜?"\9¼è?ïv¸Ì˜R?‹E˜šÓñÓ?‹âQ»«ß?‹E˜šÓñÓ?ïÿÆ:Ñ&>ðÃ!1Š">>üâ"ìœ&>ðÃ!1Š">?ïüd|£?>$'ÕÅ:?<ß-¶v?>$'ÕÅ:?ï7'‡ao?©Û KʺÁ?™Ýò(?©Û KʺÁ?ïsè/²R×?ŒGFq›§?''úF	1?ŒGFq›§?ïý/hxdk?7÷LG¨Þ?6"»3á2?7÷LG¨ÞAGN3FGL J1434.6+1951@5`àЏÐ@PS ÒH7À:0qŒ4VIÀ;q°-YÕ^¿ùu¨6À[@RÆ ‹;@ûõƒ¥¿æj²Y¾¿æ×Îú_¾=¿Ó篧"Y¿êR êNqAGNfsrq@¢ÿE8ï5PowerLawOQ 253?ï÷O>¯œ?gݞè¡1C?Q`ß^äØ­?gݞè¡1C?ïßôQ¡w?5ˆ‰72?p×&H?5ˆ‰72?ï0‰¸Ùƒr?'Õ+MU?™îÈè?-¸?'Õ+MU?ïÿÜ©ò­>æÞÛ§h>ñû–z™Œ>æÞÛ§h?ïø¡4v1é?PùZ8IŒU?M{/5&w?PùZ8IŒU?ïk+4ê ü?žF÷¡'ÔŒ?'š™_<D?žF÷¡'ÔŒ?ï"I¦ð£?"凊¡¤Ã?žm–Ò#?"凊¡¤Ã?ïý|%#…?4':6ZØb?4ؐÃ*?4':6ZØbAGN3FGL J1435.2+2023@6¬ ŸGX"@PV³`<ÎÀ9µc¾yåÀ;ByÙె¿ñõ[YBœ@
3oЍ@oU ›k¿çž3däå¿æè0-¿Û¡O–U¨¿ïÿ«mâgAGNbll@åt¢3œPowerLawTXS 1433+205?ïï'iÏ|€?fdR)‹q:?`m–[¨B?fdR)‹q:?ïê&¡¡È4?rš
êDz"?eÙ^žÐsù?rš
êDz"?î
lÌ8d?œ2JX<"?¯)?~ðöÎ?œ2JX<"?ïü"´}J®?.QM\JŸß?;bZGß±?.QM\JŸß?ïÅ·CÅôä?ŠYÌçóÆ?}$^;Bù?ŠYÌçóÆ?ï8šòùËø?§=®Å?˜ì¡›Ÿ?§=®Å?ìÍ
ó ?¨WðÅ'ü?¹—¨dÎæÌ?¨WðÅ'ü?ï¹±~+˜Ï?€%: ‰º?" têJ?€%: ‰ºAGN3FGL J1436.8+5639@Xp6ßû}º@K'ÿyÈÀ9÷ ·›`À;ì±AV¥?éÜ»¤¨¹@ïçÈ{¯N?ÿÂ\@©õ¿åëÌ´¿ãÈ|µLs¿Öf÷ŒO?j¿ÑPíè®ÞAGNbll@¤Z¾vÈ´9PowerLawRBS 1409?ïþš æÑ?$`6Å蘷?&Uî ªÈð?$`6Å蘷?ï¹ ­¸Ø?Ž¿¡bˆ,×?—úb¨/û?Ž¿¡bˆ,×?ïâ؈¨ì¯?`‰Ç7?m'wcqèó?`‰Ç7?ïp§™?'<±|[e—?œ®Qð4F^?'<±|[e—?ïüª=*ØÇ?6ÚƄ˜ç.?:®ðRSq?6ÚƄ˜ç.?ìÑNDU?»%#¸Ø?¹weŒ'¿W?»%#¸Ø?ï°"_Ùâè?ƒÇÍÁò…?ƒ÷gúø?ƒÇÍÁò…?é¬Þ öß_?¶"·2íÏ7?ÉL‡|$'…?¶"·2íÏ7AGN3FGL J1436.8+2322@=ÔW?ö@Pzd_ûéÀ9׎¢Å'FÀ;¸"lá«¿ÔxlÀ?9@ï¾v@B½ŸˆF
¿ä*Ic4¿ç-žÂ+Ø¿ãL:'K¹¿à§Á^&sAGNfsrq@Žöě¥ãTPowerLawPKS B1434+235?ïÿp29…?ǜƒü–?ù´ä?ǜƒü–?ïÞºä[Î?©W‡
k?pþ"Œr@Ç?©W‡
k?ïí›^G.?a$ÅÀ<¾F?bd¡Õ|B¢?a$ÅÀ<¾F?ïý€'œjô?  ÏFrŸ?3þÃC#ÿ®?  ÏFrŸ?ïÿNJ…'?ªè¯‹?6´~‹P?ªè¯‹?ïL0à?©GLm1×?–~™ãìN?©GLm1×?ïÕ\1†0?wÛQÏõY?uQç?Ô?wÛQÏõY?ïâ²YÙæ?fòùnƒ?mM¦=wGö?fòùnƒAGN3FGL J1438.7+3710@OÏ`?Û¸"@PQɀ2WÀ8¬N¡MÃÀ;¤ÖR5W?îÅ9oý@k0¥F@êÆ?iøA¿ã+ñÍ[¿æwè­0­Ð¿â'^³®\Ž¿ì÷=Ûû
AGNfsrq@ƒU4êKPowerLawB2 1436+37B?ïüçD¥Ôï?2…mš'¬?8Åܙ¤¦p?2…mš'¬?ïæ,I+r?u=,Å֚s?iÓ¶àÏ%©?u=,Å֚s?ïžîëåÂ?zf>`Suö?ˆD{s؃©?zf>`Suö?ïú§òç'?1jb«»?GÍ_÷èւ?1jb«»?ïý8ôN'*?=¶µ)9~?68^,vO?=¶µ)9~?ïR=žn{? T6?a}?•¸L7;*£? T6?a}?ïd?a·!Œ?/iÀ‡ñ?"xÂ<–'?/iÀ‡ñ?ïñx¨Ø?X ŽØ'Ýõ?]þÔʅ¿?X ŽØ'ÝõAGN3FGL J1439.2+3931@Q2Ü¿ôw6@P²-LiÀ9ç:Þ"_¦À;Ÿt´*¿üBÊry]@Ѐ:øÏ_?üU«`@‡…?Ê^ɼ–ò¿Úä^ä¼ØŽ¿à†8<B·œ¿Ð›¦G"AGNbll@­"Ü(õPowerLawPG 1437+398?ïþÄ@·*N? ™ÌZ7Œ?#»õÊçñ? ™ÌZ7Œ?ïâÓ[ %ÿ?€·S.ƒ%?m,¥ÓÀ­?€·S.ƒ%?ï֊ÓÙ•?oϋ"];R?tº–.J);?oϋ"];R?ïÿøBhҟ>Êc<¯ˆY>Î÷L'»‰¡>Êc<¯ˆY?ïüfÁ°º?9³\'gê?<ÏØ9'¹=?9³\'gê?ïRÆá·|?þ§í»¡?•¼Ç'8¬ƒ?þ§í»¡?ï€ÇiqÄÐ?Šzý'¶}4?Î%œ¯"&?Šzý'¶}4?ïÿ?¶N[-? Ì1¡¬ö?	<5GÓá? Ì1¡¬öAGN3FGL J1440.0-3955@tIñQç@2X&NyáÀ:MJ4¸À;¥÷T_Ó¥ÀrƒSÜöæ@
¨Ñò%¡Ð?ýÒ
ÿGv?ïZ–¼
6¿ëê%NÝÍj¿Ù#N§ƒ?R}!$#1AGNbcu@¶‹Ô¢3œPowerLaw1RXS J143949.8-395524?ïþ‹ñ1ÓY?%âc^D ­?'@í|¸ìÕ?%âc^D ­?ïÚÜZŠ?vR."‹›Ù?r'Òõ‹ªê?vR."‹›Ù?ïדGÎ~[?rH¤Bь?t6\#¿'E?rH¤Bь?ïÿÿMÂDw>•—¦Wï>–K^By'®>•—¦Wï?ïþp";—?*Å	ّÕd?(ÿtž¹â?*Å	ّÕd?ï.0Ïx:?­mŠdK?š9æÕN»?­mŠdK?ïË%n_À@?}'¾ýŒùD?zmHêìÓÁ?}'¾ýŒùD?ïÿò¬¸ã¿>äãøD¨h>Ú¦YµKö>äãøD¨hAGN3FGL J1440.1+4955@UûÐÓ@M•ƒßóðþÀ9¹[O7À;ó¼w¯d?Õx æ³"@c0¦æß@Ð^à
AL¿çuµòžK8¿è®€9²d}¿å åõ"¿Ü+µ×NJAGNbll@€_þBZîcPowerLawGB6 J1439+4958?ïþZ
'º?:½ƒéÝ3¯?*_)*‰?:½ƒéÝ3¯?ïÐÿ¾ÞïÜ?ˆáCCb?w€ 'çéÊ?ˆáCCb?ïÕñåœ7À?iL
È?u
='Ì
?iL
È?識¸é§4?mÅîòö†÷?†ÑÂ&–ó?mÅîòö†÷?ïõôÝÑÆ ?Z–
f¦˜R?TDÂ'.z?Z–
f¦˜R?î-€F¿à‰?µœõ«©–±?­'û"÷s?µœõ«©–±?ï~+mRO?ŽIՒíN?:'M?ŽIՒíN?ëvùz;¼?±«g¶îJ?Â$©?±«g¶îJAGN3FGL J1440.2-1538@uÃ?…Q
@Cßcߣi&À9§%?TªÀ;ÔCéd?ÔGÈÛ?p@¤BQ3Na@¾@—õ«¿ÐÆqO3Ö¿étÖޕïb¿å _ƒÉ"É¿âÑ,¾'ÅAGNbll@¡¸†YJõPowerLawPKS 1437-153?ïý«'áW…?3B)&­?2£é-W?3B)&­?ïÎašØ;ž?'SþK7Û?xÏ2˜±¤Â?'SþK7Û?ï«âòS-?¢ˆ½¾ñ?…Cn©PÓ?¢ˆ½¾ñ?ïÙÀXÇ?U3•øˆ?sóc`K?U3•øˆ?ïûojŽ>?F%å'?BCú¤ñ9ª?F%å'?îšre*Ú¨?²¤F3g¡Õ?¦XÙª¾ ˆ?²¤F3g¡Õ?ï==(L?˜ŸÚ>3ô?ŸØ_6£("?˜ŸÚ>3ô?îj%yk.?•'Ë¢ˆß?©]®*ý?•'Ë¢ˆßAGN3FGL J1440.4-3845@tR̟¶M@3ZŽà3·À9ÔuðG%XÀ;gš'Í¥:?±Â™¾¾¨X@Úf¸ñ£œ?û±^ûãç¿ïÏ	XU?æ[éö±Ö/¿ãè_ zù¿¥{1‹a·AGNbll@º'  ě¦PowerLaw1RXS J144037.4-384658?ïü—9åKk?HäTTZ?;F/Š°®´?HäTTZ?ïÉÿ…†½?‹"¸æV[?{=XÎ<×?‹"¸æV[?ïɌ@ô ?{	@T?{9ߏ'¼?{	@T?ï÷ñ'}
?A5¹j5*ô?Pú‹ Šº?A5¹j5*ô?ïô~XºE%?S£ë`Åjh?WN"·•?S£ë`Åjh?îÏˍe6n?µÑú'¬\?£G'ôË?µÑú'¬\?ï¡lLbì?‡jÍ©@«—?‡¤ìõ;tÙ?‡jÍ©@«—?ï¡~4¹E1?'Ðßó?‡ r؍ëÔ?'ÐßóAGN3FGL J1440.9+0610@vq[«–ò@LKT´FÀ9<¦9»±À;–g¼§»›?á¦9xzBÅ@Ý¡ejè×@úEà4Ä¿æG®)ôp*¿åYø/|¿ßu`Ôí¿Ø–Lgâ'\AGNbll@'X¢h	ԕPowerLawPMN J1440+0610?ïÿÖS֎9>òîØ?TÌ/>ôÖBô\>òîØ?TÌ/?ïЁ~+^?.Á8¸æã?w¿@íçì¼?.Á8¸æã?ïáÅi£?qåîż«v?n:–LÈ?qåîż«v?ï琐œ!?J>ƒá~/]?hop2½v~?J>ƒá~/]?ïÿ̓èµ>ù†€–>ù>&òà>ù†€–?îöSêkvÏ?«>f->N? šÁZ$z
?«>f->N?ï·ª»¢Om?ƒÅW™4;?'QîÐ?ƒÅW™4;?ïPžƒÊa?ƒ_M÷'gã?•ýl6eëã?ƒ_M÷'gãAGN3FGL J1441.5-5955c@sÅ>€8Ÿ"?¨{϶ŸQÀ8j3àØŒÀ:5é$h;?ñâãd"Ó@…ÝÞÂî}@x*.¤¿á£º"ˬ;¿ß_[61•¿áû Ôvd¿ç/z¬nˆtOTHERspp@§LŠ~ùÛ#PowerLaw$?åîm8'˜ž?̏VٚTn?Ô#%ŽÚÎÃ?̏VٚTn?ëñx¨)Ì¥?Á-õò
?À:_XÍn?Á-õò
?åö6¡°ê?·ªf¤…?Ô"À¼ž+?·ªf¤…?ë÷ˆ7 ?"§×Se?À#ß#'€?"§×Se?Օ™a\Þ ?ËPô±¦ô?å53OQ°?ËPô±¦ô?Ñˋºïæ¾?ÅæËN{Ô?ç:"ˆ¡?ÅæËN{Ô?â›'lð2?·á+=?Úɱ&›É?·á+=?àaq©²ãº?°±²ð È?ß=¬š8Œ?°±²ð ÈMIXED3FGL J1442.0+4348@SC8€®@Oû¿ÿ^ðÀ:R@|ÇÑ»À;سc$"?ìȨƒu@
µ2g±??üyvèÀ¿íÖÚâå?¼Ñt|S¸¿­).ˆª¿ÝØÓ+ò³MAGNbll@®ëOv`PowerLawSDSS J144207.15+434836.6?ï÷l¯;þo?OÚ&*C-?Q&¡dG2?OÚ&*C-?ïŽò}¥6?•ü
pðœÏ?ŒC`¡LC?•ü
pðœÏ?ï©‹ &ˆ?'Ošûˆ6?…¼Ý;eùÝ?'Ošûˆ6?îóË@}!?†Û.4QÞ? ÃK÷RÆò?†Û.4QÞ?ïîSZEç?_š =:Z³?a¬¥ËÑ?_š =:Z³?í¼â¸¶.?½¸¨ãQ?·òë5?½¸¨ãQ?ïqf¬Ì?–J'$©MY?œñÜs*f}?–J'$©MY?ìउÑi?°Pú§Ü†?¿xúÛ±tµ?°Pú§Ü†AGN3FGL J1442.6+5156@V· '½´@LÌûÆnåÀ:ÙPÑÑÀ<™‡ûâd?åG»ÞgÿÄ@
q¯ 5w?þ–?ïX¿ïýÓٗœ¥?ïÂpdÞÁ¿ÐͰý뚿ê8Te†(AGNrdg@©†=ó¶E¢PowerLaw3C 303?í:ÙÎE¦[?ÅÃ,ê2¨
?¶)1Œÿ+?ÅÃ,ê2¨
?ïÞbï'?¦5IM{ÞÉ?ž"3¹'s»?¦5IM{ÞÉ?ìÿHv!«ˆ?¨8«"p&à?¸¼M:ÕÆ?¨8«"p&à?íj-g¹š?Ÿeߙ2_†?´®"ÁWH?Ÿeߙ2_†?ìTŝ¿ª6?Á)ótèp}?½YÓ®S?Á)ótèp}?êÃü̙Ì?DŽÏî¨?Äð͘Ϛ?DŽÏî¨?êà‡D,»?³ÂÙxB6?Ä}âïN?³ÂÙxB6?å\&7&?QrÓ ?ÕGÛ³'ß³?QrÓ AGN3FGL J1442.8+1200@ ¸G '¨;@MéšÑVŸÀ9±Ú/‹ÞÆÀ;|1u¿ãy:M¦ƒ@^ŠPPzl?üºlà¨÷°¿çyqcªÌ¿ÛvI³ç¿Ä\qî¸b¿Ý¼ü'.¸AGNbll@­ÚöE¡ÊÁPowerLaw1ES 1440+122?ïý²/½‡à?0%Gæ—þ?2n‹jb?0%Gæ—þ?ïåÑÇn¥5?yuw; î‡?j.8[Àâà?yuw; î‡?ïÕ Ò­À?u¥•òäBC?uoõê°?u¥•òäBC?ïþÇ_"Sù?ÃÆIvmª?#Š~ ç?ÃÆIvmª?ïûiß'ÿ_?<Õþ°ñ–
?BXƒž!Ûb?<Õþ°ñ–
?ï5>´m°?ªÒ¯iNH?™X-í?ªÒ¯iNH?ï½^@ŽKÄ?Â!‡>9?€¨oÖ=Ã?Â!‡>9?ïõ"}a:ê?S¸Õ4'z?T×[Ƽž?S¸Õ4'zAGN3FGL J1443.9+2502@AKy@]¾!@P,rßñl¿À9D–¸=ɏÀ;š÷Ÿnd¿â/	Ì@ø¯.+aƒ@V¾|'¿àEËE…'ž¿æ(>Yú?¿Ô!Ë4yã¿èKŽÿaÊAGNfsrq@•û…‡"ÞPowerLawPKS 1441+25?ï׌¡c'w?§n›~ª?t9¯_dР?§n›~ª?ïã½`¯S?ò‡¥
?l€B{"¼¶?ò‡¥
?ï¤ÛÄ·T–?…mØr2҄?†ÉÇÜ­?…mØr2҄?ïöèþlé?B^™	Š‰r?R.‰""4?B^™	Š‰r?ïó'…ƒb?a54›ºE?XÚõ…ƒÝ"?a54›ºE?ï:Œ_y?¨X®Br?˜®}-1¤X?¨X®Br?ïI"¹Rê?"iû0eÂ?–Í~®8Í?"iû0eÂ?ï"}bC¨?‰×ÈVm
?Žà»A
?‰×ÈVm
AGN3FGL J1444.0-3907@tZàP7P@2¸ßh°ÄÀ7ó¢²G‰À:¶³žþ]i?ñß°	´A@æˆ*?üùë`á—4¿ÞAPb#¿ÖNÏA­Z¨¿×`·-†Ô¿ÙÚX³5€AGNbll@¥Z…‡"ÞPowerLawPKS 1440-389?ì?'æ¬zz?Ã5-uüRï?¾Àʜ,,?Ã5-uüRï?îZ3®
óW?¯E‰ Göž?ª\Åtã–?¯E‰ Göž?íyGžÇxG?¥û¨']?´5ÃèVÍ?¥û¨']?쏬ÜӑH?—97é'8u?»'™cu¾?—97é'8u?ëžÕø3q¶?»"hñ
ÒY?Á"¨29'?»"hñ
ÒY?ãÎÜ=ûZ¡?ÐÑp´âº?ØbG"	J¾?ÐÑp´âº?ìx~bAÐ?¨Ž…d9'±?¼?<íñ'?¨Ž…d9'±?â¼MÏ'?¶Úyd+3ò?ڇda±ÿ?¶Úyd+3òAGN3FGL J1445.0-0328@uÓ1ŸŒ¨@HuËCòžÀ9§ËtÝøÀ;p	{¸¿îÚœ"ê@,"+ž>o?ÿIØÿ5)Ø¿á,š¾ÃÛÉ¿Ù0õÿ~®d¿áºì¶)м¿ÖæÏ7—OAGNbll@£›
~ùÛ#PowerLawRBS 1424?ïþ'˜&/?"%/gTxÐ?&Ö}GC ·?"%/gTxÐ?ï×{•±?;ÙG?txBj¶g¾?;ÙG?ï×çkš¾ï?qÉU…ØÆz?tJs¼À?qÉU…ØÆz?ïÿ£Ëeˆ_>ù°4?J³º?
'«ò·>ù°4?J³º?ïü}ãkÛ×??Æ6ß?<ã%ÌfÏ??Æ6ß?ïUŒAu¸?§ÚfÌê^@?•Nwä€ï?§ÚfÌê^@?ï©`ô¦?…à¦9a?…¹û ãžw?…à¦9a?ïù¹‰ûÅ?DÖ	®˜
/?IÚ¦I§ç?DÖ	®˜
/AGN3FGL J1446.1-1628@u,ù jn3@C$CÀI0ËÀ9á·äkOÀ;†­âü¹ú¿ìùËVÒ@¾…Mi@ßy_'a¿èA5Ø)!¿ã†È1:=F¿âÛåÍ¿æªÔͦ^AGNbll@'Sݗö+PowerLawPKS B1443-162?ïý.ŒãÜ<?=4¨B)Â?6‹–ÊÁM
?=4¨B)Â?ïÒÃð–fÅ?Š†/cس?vž¯ý)P?Š†/cس?ïʟg}¬m?x½@u5– ?z°LU…j?x½@u5– ?ïýôޟï/?!<"vPf~?0Y
¥¬?!<"vPf~?ïôèU¥Š$?Zßó'ñ?V/TT¶¨®?Zßó'ñ?ï-J!Ðùò?©ˆ•tÍ°˜?šV»ÉP]¿?©ˆ•tÍ°˜?ïCÆü~@M?'÷'—HÐ?—‡ qïÄd?'÷'—HÐ?ïÒÛ2|e=?r›õÓ)æ?v'fÅìéº?r›õÓ)æAGN3FGL J1446.6-4701@t(Óõ¶@&ÓÈß'·À9äþú2À;]Ê÷àvÎ?ïû¶' µ@xߥA˜|@bÏߦÄ%¿ê Ð]â¡¿Ô+ÿÊrvâ¿äg=› ¿ïþ¤&Kª_PSRPSR@ó´êJŒPowerLawPSR J1446-4701@?äòókXNÝ?ÏT}TX`®?Ö)ObF?ÏT}TX`®?ê§+ebI?Á6±sf:X?ÅcSÆjvÛ?Á6±sf:X?è҇=eU?¯²š?³~…?̵ã
j«ß?¯²š?³~…?èn½4÷·?¡îtÁŒÁ‰?ÎE‹,!$?¡îtÁŒÁ‰?Ô4VGÏc?Î!jš
îç?ååÔÜwÏ?Î!jš
îç?Ù
àØ^?у.d'®?ãy"úPò?у.d'®?ß.ui
µ ?·ÙÒã2?àhÅKy%0?·ÙÒã2?ÏEÿHuË?®âKBíÜ?è.€-â¼M?®âKBíÜMIXED3FGL J1446.8-1831@u••:@B:)@k*À:q?8$4À;›Ÿç't1?ãU4%‡µ'@
¯–§w?û'#¾Ì#?߬$Éì{F¿ï'Hˇ
·?î¦ïc"¿Ó±²ÚÞ2{AGNbcu@º/î¾ß¤@PowerLawNVSS J144644-182922?ïýÙoG‹…?8Ø.˜ÚX?14"/?8Ø.˜ÚX?ï¸ïТß?y*Ÿwg?Ä=Ùí®,?y*Ÿwg?ﮅìéwÓ?ÿx,ʱ?"^"Í1/#?ÿx,ʱ?ïØœéý?mQ©n
Ž?s÷1v+í¥?mQ©n
Ž?ïùmÞĊÎ?Pqe¤Öj?JH"A56Æ?Pqe¤Öj?î!\åš_M?¼Ø)LT—?­ê1¨íÀ%?¼Ø)LT—?F­¨3?‹ɬ¢Y?Ó.[u+,?‹ɬ¢Y?ォÅý6?Œk;:Ó5~?€•‹R?Œk;:Ó5~AGN3FGL J1448.0+3608@N"ˆ?Õ%@OÛ¿[o'À8߉çtî¿À;;Ɨ(¦?Ø9scÏÞ$@×vôÓý?ý%ßbц¿Öã"8'þf¿Ùïw`x‡¿ÙAúÚ.è©¿ÕñÆOÖAGNbll@£¹"MÒñªPowerLawRBS 1432?ïþoXõ±ë?K÷&}Têz?)
oôõTê?K÷&}Têz?ïà †Þ+?Œtb8tà?oßyP–·?Œtb8tà?ïØÀ¬5±?vR¤¡bK\?sŸ©ð&2¸?vR¤¡bK\?ï÷¢Õ=ÅÅ?7I,Æó¦Ö?PºUíF¦?7I,Æó¦Ö?ïþ÷Þ.°(?ÄA0QT? 'Ñ\†m?ÄA0QT?ïUΐò++? 9CR?•F-ẚ›? 9CR?ïÚê9^?yŸuz8?røý"ÒLï?yŸuz8?ïÔè=|Ée?l2*ñ?u‹áMIù5?l2*ñAGN3FGL J1450.4+0911@ lŸædÎ@LUÁ HàDÀ9íþu¼D¿À;»˜õ.릿éFïþ€#@
Ç+Î@ʽ`s2R¿æ°²ë$P¿ßt ×·¢¿Þ}®±Ù¬Y¿ì6ʸ(-¤AGNfsrq@'­jçÕfÏPowerLawTXS 1448+093?ワg¡œ??ƒ¸cö×ݬ?€Xæ
úV?ƒ¸cö×ݬ?ïàΖxä?=X&7ò=?o1ûOj'?=X&7ò=?ép®?˜½pÑûë?¥•6#üª"?˜½pÑûë?ïþ{ýÁ%>?êõÑy*¯?(@&vbc?êõÑy*¯?ï‡×6ªƒn?•©"Ñû°œ?Ž
2_­øg?•©"Ñû°œ?ï-[6®?ªÄhCC?šTŽ!ÁEÛ?ªÄhCC?î;!J—A¿? @Rù9–?¬MëWgË	? @Rù9–?ïîeAD»?^\Ð-äo?aùš¬ÝLÛ?^\Ð-äoAGN3FGL J1450.9+5200@VGŸõÔ-@LF{ÓöÀ9Á
Ìq]:À;¿bÀ¿xP?ða#""@7_a@k=ŸrÌ{?ïåq Ã^¿æ>Ölá¿à.Έ°=¿èŒÚWéÀAGNbll@™'ˆðŽPowerLawSDSS J145059.99+520111.7?ïi¼O;?½2o‹J˜Í?'ÏÈw·?½2o‹J˜Í?éÈ%¹€R?ÉSê$˜Ýÿ?ÈßiýŠ¸?ÉSê$˜Ýÿ?îò<K=s²?•Z¼5¼)°? Ü;N¼yä?•Z¼5¼)°?èËBÝäæä?©uŜ/`?ÌÒôˆldq?©uŜ/`?ïÏ1ÈòD"?€­†ärÊ:?xggñs#?€­†ärÊ:?áêÔIÃÃ?ҞV‰	æ?Ýà*Wlxy?ҞV‰	æ?ëê
iÂ?°m(dõŽg?ÀWï—ÊX÷?°m(dõŽg?Õ¾ýc:~?·}3iÉN;?å NbþA?·}3iÉN;MIXED3FGL J1451.2+6355@Yæœýç!@H;ô|ôÀ:ÌVô›¼À<,SÐa¬Ã?Ï+$]¤Ã;@ÿ˜_ݶ)?þ°Á(~Ï¿í‡t[¥ ¿ÅíF挎¿ä¶ˆî¦'¿ÎùƒÆëÙ¥AGNbll@°%Pÿ—$tPowerLawRX J1451.4+6354?ïà®Ç[ÒA?sšn{"¾?oQ8©­š?sšn{"¾?ïÛY'J?ƒ'¬ÄPÚ?rS¢+GY?ƒ'¬ÄPÚ?ïHSÍÜ|?"Wbn]vk?–õ†e›vz?"Wbn]vk?ïàêAŠ²?Z¬ãß4†?o¾úv/?Z¬ãß4†?îÎtÏØ?¦´/ûxå?£8²&—ê?¦´/ûxå?E¥?±2œ º>8?¤g¿™íÙ5?±2œ º>8?îÄ¢yßa?›à2áý×?£¾ÛÑ¥ä?›à2áý×?î+H0x÷@?£ý6cH·š?­K|ùLrú?£ý6cH·šAGN3FGL J1454.0+1622@2Œqà,l@MÖû¿ÿ^ðÀ9øNz·VCÀ;ÊmÍÓ?¢]‰3ue@@ם¶3Ù@¿‰ÿ¯~¿ä!¶"F摿螓è:ø‹¿äNþC^Ç¿ïÿïÛ*ï©AGNfsrq@'ƾvÈ´9PowerLawCLASS J1454+1623?ïÅ¡(ò´?•Žq¹jë?}/k¼µR0?•Žq¹jë?ïΠÑ5+?'x5XÂÝâ?x¯—}w´s?'x5XÂÝâ?îmyŠÛeÂ? ´"`@÷0?©(gOµîç? ´"`@÷0?ﶰ*L&A?hà¾7…í³?'Sõ}™¿?hà¾7…í³?ïòÇ,ú´ç?e¯ó5áË!?Zq¦TÍÀ?e¯ó5áË!?îŸ6ºãQ…?´Þ5²—Öò?¦"P·?´Þ5²—Öò?ïm@äæc?—œ3 î
?Ÿ2Wãc3£?—œ3 î
?ì‡8g
âB?¬j{m
z?»Æ<Ǩíí?¬j{m
zAGN3FGL J1454.2-3751@t'Ž wm@2ìïÔ;VÀ9R¤ÅFƎÀ;qÆ:âT¿ò7wÀÖÊR@ks]oǹ@ Û´¿ç6üºavy¿è×{È´uy¿îs€Wÿ}¿ÉYSæ(ŠÛAGNfsrq@z‰-à
PowerLawPKS 1451-375?ïú§-«ßÂ?S™ó¾±y?EcHƒþžc?S™ó¾±y?ïÐèî@è?‹Lr@܋~?w‹ˆÞX3÷?‹Lr@܋~?ïÃlѺr?…zÄÕ")ø?Œ$IJ+t?…zÄÕ")ø?ïÿÌ´ñ>ôq
æ¾>ùõ©%;Û>ôq
æ¾?ïï0æìw|?g\DÚ¤?`ÏÔO´†?g\DÚ¤?îÿÀÍÿÂ?²àÁ¿±? £õ³¸ä?²àÁ¿±?îäº2¸±?—•à½Êš?¡¾d[øì?—•à½Êš?ïøÈõbÿ:?N‡LËí?LÜ*6oN?N‡LËíAGN3FGL J1454.5+5124@Uêx $Î@L9o¿«|À8W!CF¦­À;IŸß-øa?ð¶zӅΌ@»W";Œ@«¯‰øè¿ße5x÷|¿âBÿ÷æ¿áï'Á;§ª¿áì6CmAGNbll@"韊	ÞPowerLawTXS 1452+516?ïÿŠ¬Ä³?muºNÿ¶?
{M8é$?muºNÿ¶?ïά'¼õ?±Œ ª…}?x©ó&ÓQj?±Œ ª…}?ïÎÐÒ.Ð<?z"~Tâ?x—–Ôª&.?z"~Tâ?ï%ê?¤Z¾?z"ûKÁ²?›B¸t¨I?z"ûKÁ²?ïÿpa'ä?ç#ñ'¯¥?ýØÍȺ?ç#ñ'¯¥?î"昌?²2ò@…É\?§¾á™æÛ?²2ò@…É\?ï°0×¹9ó?‡æ5À
2?ƒóÊ ß1?‡æ5À
2?뿝Zfå?¬DõÅV›?Á‰¾–dl?¬DõÅV›AGN3FGL J1457.4-3539@tž5 ÝD@4‰4ŸCý†À7he²â?üÀ:ç·I­Èü?úMÔ§6»(@D}Ä&
+@\'eîqb¿à
´5Òñ¿å'Úák
¿äã\C«Y¿è'Ÿ5ÁOAGNFSRQ@}âÕ䣃'LogParabolaPKS 1454-354?ï÷a+F³K?PiíwÆÄÎ?Q=©ùJ§?PiíwÆÄÎ?ïÅ
wÁòB?'ÆÊÎF©Å?}zÄ&–ê?'ÆÊÎF©Å?ïžÀLƒ3?"MO¥—ò?ˆxÏéo—S?"MO¥—ò?ïþâvພ?÷Î$çÐò?!ؕ"õZ?÷Î$çÐò?ïôÇ
Y?S¢Œé¡h?Vqå4G'V?S¢Œé¡h?îÎ?͏.K?¹tþ=»Ï?£#\?¹tþ=»Ï?ïPíä} E?'«ï¦yMŠ?•âCs˓b?'«ï¦yMŠ?ïÿmÓË¢?éؔ!=3?rAº"Ø€?éؔ!=3AGN3FGL J1458.7+3719@Në<¿£ï^@N°q?Þ<aÀ: –Ϻ¾À<DðÊØ׿È$=Æxä‡@¨ÜRPÚ¹@êvjG¿äé¯z<Ã;¿äiÏ°""¿çñԇðé¿Ûœ–½àåwAGNbll@˜ýa|ÚQPowerLawB3 1456+375?ïþ…ŸšB??-¹¸I½K@?'¦\f•?-¹¸I½K@?ïã\X6?}wnº0‡™?l£¨³yÈ?}wnº0‡™?ïþv¦X"?uQ)`Ó?~ ÄÉ»?uQ)`Ó?ïøC}ÙÀ?9Ƀœ¶Ð?NòâüàÎ?9Ƀœ¶Ð?ïùõfé?P>ùmã£c?H*f¼:Ã÷?P>ùmã£c?ïEDÓ?Ÿr©ºOu?—\^X-ž?Ÿr©ºOu?ï	IR·æi?›-M %?žÖÕª»Ò?›-M %?ïo@¾ûÃ?DLg?'ä°ë±?DLgAGN3FGL J1459.4-6053@sÞ
?‰'Ë¿üƌ µ,GÀ6íF4—·AÀ9ûÏÑdB@hzn±@
E\-}@¥€
¿Ý¹›¿änì
Än¿çÿP§Ë¿î¶œxŠðPSRPSR@õØy=ÙPLExpCutoffLAT PSR J1459-6053?oY™S?
ÙwD
?ïÿ£–?‰?
ÙwD
? Yw‡ÏV?»ŸÁj²À ?îÿºhyě?»ŸÁj²À ?š@ï ™.Ž?™?ž)?ï-ø†íx?™?ž)?nÀ'Ÿø?W-å-þ(W?ïáê?=Fv?W-å-þ(W?¥÷ŒÖ™?_tÝ"?ïÿB×QFU?_tÝ"?…RD4Q/6?©¡´Õ'Û?襁ï.»C?©¡´Õ'Û?…|kÑÙRÌ?½±±ˆb?ïªPÕ?½±±ˆb?:K%±U##?3öÚK?ïü¶›Zü?3öÚKPSR3FGL J1500.6+4750@TGŽÿâ£Ï@L¸®Ú«³À9þÁqN÷µÀ;t7.jv–¿çVjòß}v@ }kœÆ@$ q¿ëŒ$œJ+¦¿ßL©_Fë¿éù"€­ºc¿åø"–ðAGNbll@ŠßuâlvPowerLawTXS 1459+480?ïýÐ[*P¿?8dÍ}¢?1}$¿Ëð?8dÍ}¢?ïÜ¥÷Bv?Šæ¤#I³?q­em`?Šæ¤#I³?ïyâ
»^ª?‹hI?Ã¾¦Ü\¿?‹hI?ïüÜ´V?)M¦×1?;!È"D?)M¦×1?ïîUuIÐ{?i¾K7c?aªŠô|±?i¾K7c?ï³fŽK?©¤ê'|ç)?œ©"6Óü—?©¤ê'|ç)?îqbngÅ?? #`~cì?¨éÙa? #`~cì?ï¯V"¦K?}|'Xɓ‡?"*|çms1?}|'Xɓ‡AGN3FGL J1500.9+2238@?pc_Jé2@N.µÀ@ÍPÀ8î÷Œ"÷™À;N;õy"A¿åŠ<ïÊ}½@é×µM?þ±J b5ª¿à'Ì!ÅçD¿Øz"ZóÁƒ¿àørOu¿ÕÓËÕzWAGNbll@ õŸ¾vÈ´PowerLawMS 1458.8+2249?ïÿœõ2‹\?3·ʀ?ÂÀY4?3·ʀ?ïä/fÂN;?j›"tQ2?kЙ'´E?j›"tQ2?ïÖ­\€DÅ?vbŒ5Y³c?t©QÊ,qi?vbŒ5Y³c?ïÿÙɬÔ+>ã
`n'>ó5£•±D>ã
`n'?ïÿYËè7?;½ˆt2õ?Ƈ0z³?;½ˆt2õ?ïj²ºÁ¡9?Ÿ¾•ªá:y?'©¨¦
Ö?Ÿ¾•ªá:y?ï×5ÅÎo©?yÆҀv£?te9Y?yÆҀv£?ïþ¿@г??!'Ê›u?$ö˲Å?!'Ê›uAGN3FGL J1503.7+4759@T;[À6ã@LvÊàc'†À9ƀÈè;¾À;›)гâ¿Ø¶á´'@ç÷ˆã@½è@EÀT¿Úªüg´¿å>¶DRÈØ¿ä—$äæÊ¿åŸGïêAGNbll@ ¯S@N¤©PowerLawSDSS J150347.99+475930.9?ïþ×0yå?&³êqÅo?"Œÿ‰5éß?&³êqÅo?ïÝØÁ~ ?"7­¸ð?qóƒÄý?"7­¸ð?ïصi¿ó\?{«ª<Méæ?s¥K,dê?{«ª<Méæ?ïûšŠQÊo?,›N äÔ?A•Ö©ó)?,›N äÔ?ïýÉY›ì?7ì| ö¹Š?1·¾"Ci?7ì| ö¹Š?ïW†.ý?©•B¶¢­®?œ5@	¼_?©•B¶¢­®?ï¢g°?ˆÊêéP8?‡{»@Ü?ˆÊêéP8?ïÄ	  +?suÚCÎ!?}ûtæ?suÚCÎ!AGN3FGL J1503.7-6426@sɛ€#¦ÎÀ–šÀ
F«À8å¢4rÎÀ;vJßø#?Û毶UUâ@­êY$´j@¦¬ l¿àjÞ|ô|¿ç«
ü÷ü•¿âÄjMÚ1¿éEpÑ4¡®AGNbcu@'§å`A‰PowerLawAT20G J150350-642539?ïû.qØ_}?DÎ;òæø¾?CF9"NPÛ?DÎ;òæø¾?ïh´·'7Ó?¡«4"{½×?'éi(¡–?¡«4"{½×?ï°¿!àÇÎ?ƒ´ô¨&?ƒÐ7ˆ}ø‰?ƒ´ô¨&?ïÅ©oÇÛ?\›Èô×'!?}+=Í>W?\›Èô×'!?ïò/"hœ?]ÀW±µIÄ?[Õ¢c×Â?]ÀW±µIÄ?믡©ïŽ?ÆJœÆʪ3?ÅAyXAÇ?ÆJœÆʪ3?îÚ÷4 æL?—úæˆ81?¢PŒ¿©i??—úæˆ81?î^DnøcÝ?¿Õ¼ŒB?ª¹Û1?¿Õ¼ŒBAGN3FGL J1503.7-1540@u|0¸,,@B?ñ7À9&M±cººÀ;*"ž­Õ'Àý¸à[Ê×@¡nu©z?üPOÞº‹¿àü᫽CÔ¿æóEkˆÓè?©Ÿº"®´<¿Îs0õÒeÏAGNbll@±néxÔþPowerLawRBS 1457?ïü˜ºK•Ö?:'ü$0êa?;:,2û5Y?:'ü$0êa?ïÞ=ê`i?ƒàÞ|úˆç?pá
ÂáÇr?ƒàÞ|úˆç?ïʦÌ̼?yM¥Uá7?zý,€ÜrS?yM¥Uá7?ïÿÿþíA>)ª¸³m	¦>!BLÆù€ù>)ª¸´Ýøú?ïúûÉ¡Ó?CTÉWŸMC?D÷ù+Ð"?CTÉWŸMC?ïK¹'ã?¨HñRÁ''?–ˆÎO–±¬?¨HñRÁ''?ï )"¹†?Š¼eIÑr]?‡õ·U*úŒ?Š¼eIÑr]?ïÿÿÞ¶Èî>€ç'ŠX†>p©ümî1¶>€ç'ŠX†AGN3FGL J1504.4+1029@&Û`C6¶@KJ0 Y;ÛÀ6"bÕ¸-ÙÀ:¨
ހ@ÀY#²·£@"så!Wh@;l0ªÂ·¿àŽ™ë4¿äˆpeSýê¿åRԐæl±¿éDŸ¶š©AGNFSRQ@u'Æ)ñkLogParabolaPKS 1502+106?ïçÄÃF™Ë?p=xÛWÚÕ?h;<«§Å?p=xÛWÚÕ?ïá£cqêS?ÍÔ^¼xí?n\œ~÷dú?ÍÔ^¼xí?ê߁¶+©/?²)Ï·VÒ?āù'Q[E?²)Ï·VÒ?ïÿÚHéÜ[>îlwò>òۓO 9ð>îlwò?ï;ÈqYš·?›ô­Ò»Ã?˜†ñքw?›ô­Ò»Ã?ïLô‹"Ø¡?§ÆÇ'âï?–an‹Íî?§ÆÇ'âï?ëÖ$ñXd?­œå<³?À§l;Ξo?­œå<³?ïÿöLof¸>Û±v&~Îb>Óg€IíâP>Û±v&~ÎbAGN3FGL J1504.5-8242@s3Y'ÿÀ4øc ¹HŒÀ:WG6wÀ;·^j¢Ž¿èìãuÃ@Í)éÞV@aÿ ^¯¹¿é³· s[¿åqµ%ªù,¿äÄÖô~E¿å/Ë6õŠ†AGNbcu@–x\C,¥zPowerLaw1RXS J150537.1-824233?ïûb }ñ??Q,Úxaޓ?Bw~*P½Å?Q,Úxaޓ?ïÎx$:?€ß+ß­Ö?xÃî
œó?€ß+ß­Ö?ïÇ]yØ´?uüYEÙ5‹?|QC	W&3?uüYEÙ5‹?ïþ8±ÕÙ?^Ïè xz?/œw "^?^Ïè xz?ïâ8Œìë"?uÔá¯å
Þ?mÇs–\G?uÔá¯å
Þ?îwVŠó…ì?¶Â«+{¨?¨Š—U$A?¶Â«+{¨?ïå¥ûk‹?•æãšߚ?œ£KE¹ø©?•æãšߚ?ïÚ¨—ç?l<™è	Æ?rÿ,â¸D?l<™è	ÆAGN3FGL J1505.0-3432@t¾¬à2Û@4³	¿œb¢À9­&|k‹iÀ;ÞŽ–0Y?ᜏ Ï÷@ ƒ™:@×ýFKê¿èäÜJÚ$*Œ¡—¿ä?[ ˜D
¿ä]cMWKÁAGNbll@™ç»/ìWPowerLawPMN J1505-3432?ï󆾆Ê?bD!úEÝ?Xòƒ§%?bD!úEÝ?ﳛ'Þ(?"ÉŠKh¡9?ƒˆöÒ?"ÉŠKh¡9?臨JÝÒa?ƒ¿¼2"­Ÿ?†m7][È?ƒ¿¼2"­Ÿ?ïw§u
ª9?k4šµÒ %?'e‰ðÐ?k4šµÒ %?ï˜B§‰ê??[Y"a?‰ïV/N±›??[Y"a?íI¹ôû6?¸À5JH?µ²0Yp&?¸À5JH?îµÞÓN_ù?œRtU¸$f?¤¢Ïeƒg?œRtU¸$f?ë5µL08?¤Xªæóê?ó)*Ï?!?¤XªæóêAGN3FGL J1505.1+0326@ä×?Âb¼@I ÷þ½áÀ8…,$K9À;p§I……?Ò	®³@4؉™q@ßú D®†¿å6}âÑ=¿éÿHÂ^¿è иØ$¿æI̧¸ìAGNnlsy1@|ÑéùrGPowerLawPKS 1502+036?ïô®Z=Z¡?dMóø8¢?V£K–NÞ?dMóø8¢?ï½À	V?~ÆӐ?¼?€ú½­–m?~ÆӐ?¼?îóU^p¥?˜ÀÃj}–<? ÊªIº?˜ÀÃj}–<?ï`Â|U«?"üÁpÈöò?œ3ç³äæ¢?"üÁpÈöò?ïÐxà*fu?Ž(ëÂÂn
?wÏÿjm'?Ž(ëÂÂn
?íÅ<‹?Âcž9UP?·Iëðú4¬?Âcž9UP?î
¾$ÿ?¡ÙRµ?¯'ä
°?¡ÙRµ?åûê$)3?¿t<gåAŽ?Ô	Æ+·­›?¿t<gåAŽAGN3FGL J1506.1+3728@NÉÍ_™Ã‹@Mò•¿ðExÀ9C×xø9À;É}»Ûä?ò]§rö@"äÀ`Ù@Ÿ+À£Ò¿áõpÙ˧£¿æ.5Lèæß¿è«øP€˜c¿ïü8—Ô¦AGNfsrq@"@'ÑN;ÍPowerLawB2 1504+37?ïõ˜´}†Ð?Pò³?TΗ0í`|?Pò³?ï|净?œr}US4)?cO°ÄÛ?œr}US4)?ïbËùàxž?ƒöBN5?"¦€ÉVF?ƒöBN5?í»T­–|?Ž?\êÿ¢?²%_LK ?Ž?\êÿ¢?ïî­2ä¿ï?fa.û'?aRÍ
ÁñC?fa.û'?í#Ÿ¥TìI?¹ý¾(O?¶ãÓ2Ü:?¹ý¾(O?îÑÜtÆ·›?šdO(ê×e?¢â8±Ü¸Q?šdO(ê×e?å{ùˈ?¶Í9?Ž?Õçhï?¶Í9?ŽAGN3FGL J1506.3+4332@R>Dàá6@M#˜ÀUÆÀ:ŒÅ½äÒ}À;ý¬Y¾O?ËV‰?•}f@
Òæ6«7Ò?ÿ'T€	û?ïð·EçÒ¿Ï"ÑžâH¿Þˆž«Ò+¿â)˜'©AGNbll@¥Iþ\'ÑNPowerLawNVSS J150617+433413?ïþÊÛRn? J&HC$ã?#RHè%|? J&HC$ã?ï×ëF«"?†"ãQ@÷?t
sp—ò?†"ãQ@÷?ïÅ -qþ?z-ƒ"Ÿ1Ó?}oéZî¬O?z-ƒ"Ÿ1Ó?ïÅ\ªØË?d ¿YBü?}Qü¢TŠ?d ¿YBü?ïû½™À±?ALi,ÒÃ?A	½A"ùÇ?ALi,ÒÃ?îñ«IQ?§¾(ªz.É? åOù³!å?§¾(ªz.É?ï†,×©?‹w'6¢>ß?ŽxtÑ{AÇ?‹w'6¢>ß?î=rõf? ²—­¶P?¬(ЭÒ¢? ²—­¶PAGN3FGL J1506.6+0811@!VèË@JiÙÁfgÀ9µ/V/À;€«rßñm?ëNÜ~h@;=‰ù=™?ýûö€¥Vç?ÅUw…úù¿àŸKã`놿Ϯ"ý¾¿àÿ{τ7AGNbll@©ùCþ\'PowerLawPMN J1506+0814?ïñúr'0Ù?\_#ël?\×S?\_#ël?ï³o Ä2?Œe±Á Í)?ƒ$Nq?Œe±Á Í)?ïXý¼G³7?'¿H"?"àHs™ý-?'¿H"?ï+@­??̍#¡ë?š—ÿ²õ'›??̍#¡ë?ïã¾Ùo˜?lµçÖÜü¶?lA&¡a‡'?lµçÖÜü¶?íÇXY2vJ?½?N	?±Å=4FŒ4?½?N	?î»WàDVz?œ"D¨šv5?¤JúÞ±e?œ"D¨šv5?ì¶tò"û5?©†	Jº5?ºLXnè&V?©†	Jº5AGN3FGL J1507.4+1725@6ëòÿf}
@L—«ßí;À:—'ï2RcÀ;Ñ<*R¹á?áËÌVÛ.@«¤íµ¥"?ü‰!ACAH¿ïê(¯k?ïšÐsÓê׿Òî0÷wN¿Ób¡éAGNbll@³";~ÿ—PowerLawNVSS J150716+172103?ïþۄ9yã?+1== v?"G¸"9{1?+1== v?ïÚC'Œœ?†"=lďÂ?rÞlZæ?†"=lďÂ?ïÆ]±OÝ}?|Q–µãv?|Ñ'r.I€?|Q–µãv?ïݾ2fjÔ?^ZÛ»p»?q æÎÚYÚ?^ZÛ»p»?ïý&L
?7ÝÄ©?7&Íug¤
?7ÝÄ©?îàЄD?°8£eüŸ?¡ò÷ÄGB4?°8£eüŸ?ï¢#ÿ—-?…äcÓuCµ?‡w$ƒ'?…äcÓuCµ?ïg–ëЄN?‹%téû ?"
">W?‹%téû AGN3FGL J1507.6-3710@t®ÿÀ	oë@2-×,uªÀ:	JÅöï¶À;Ÿ{Òuð?Ì1kKÂ:@
«$õØ´¸@jßÇÑ:?ºWZ€Dl¿åH¡y·Ñé¿ÕT…ࡍ¿æ…ÛÊý¥ïAGNbcu@ Ë-úCþ]PowerLawNVSS J150720-370903?ïýÄècƒ?1óH	J«Ç?1ؽ†áØ?1óH	J«Ç?ﳌ;PÊ?š?DŒŽ?ƒùxk?š?DŒŽ?ïÙ6qE?m"»<áÆ?sdÇK¡È¡?m"»<áÆ?ï±h'Ó–Y?dT	«/¼?ƒ¥Ûš§'?dT	«/¼?ïúîϒ52?Dó;z?DDÂP;²?Dó;z?íõ0FwfG?ºâ.!À2ú?°V}ʌÿÎ?ºâ.!À2ú?ïÁ-¦ù ã?'Sž(BÀú?i,p¡ªÁ?'Sž(BÀú?í÷ܽR(?ž ˪ÈG?³A§{B?ž ˪ÈGAGN3FGL J1508.6+2709@D€"ð½@MÈ÷`MÉÀ:YÞ9ÛÀ;³¤ës¸¿ÐŽïnYÇ>@
2ôU¿?ûXt@Éп圏º•¿âj­…+Dõ¿ÅÌò—mx¿Îå}éÃ[AGNbll@¹nBZîcPowerLawRBS 1467?ïþÞɾ>X? o+õùfÑ?"c©ÁG? o+õùfÑ?ïÝð}õä?'>¬hGIè?qÁ^gf?'>¬hGIè?ï֎	Bžá?tÌk—jw¾?t¸ûA#ë¨?tÌk—jw¾?ïýžDŠYÇ?!@œN*wí?3
܏±¡§?!@œN*wí?ïü4ý@e©?>HZ¾'1ÿ?>XžCÜ?>HZ¾'1ÿ?ï^VØÌ,?›'ÎÀû§?"?!vމ?›'ÎÀû§?ï¥K3Z†?"™ö¥}p?†­30WVk?"™ö¥}p?ï뱘$4Ï?aa#i8?dNgÒ,I=?aa#i8AGN3FGL J1508.7-4956@tF7GMœ@†¿ë½ÔÀ8¥ïm
ÅVÀ:ô"Ýz™ú?ã;Rø¸@C4LbÚ@Ø!¿˜[׿çßsâ3¡¿é÷ž€f˿筕~g1¿èœpc•QAGNbcu@|~äâmHPowerLawPMN J1508-4953?ïþb[ى?.V3ऒh?.™Þ^
ê?.V3ऒh?ï"Vc?""uN}êÑ?‹*®¬"V?""uN}êÑ?ï€Öl«?ˆ
,vF&'?ù
vE
?ˆ
,vF&'?ﬕùb=H?d[#·Ÿ$?"ځªàIô?d[#·Ÿ$?ï÷bb©K?T‰ÂNØ?Q;:úa	w?T‰ÂNØ?ìƒÂa}¸?Âú
¦2?»çùìô??Âú
¦2?î˜Dœf0?œŒiâ1?¦{¶"Ê?œŒiâ1?íºñê#Ü?šq³Ê½ëî?´(qŠÈ ?šq³Ê½ëîAGN3FGL J1509.4-5850@sÿ?á—_¿ãÄ&½ò·À6ÿ\£oqÀ9ê÷ãÑÌ@äª1xg@¶'ž?ý˕/&´?»Í}þ'¿ß!]
ÞK6¿äÀj4À벿옗A‹Ì¹PSRPSR@•ÿĵÜÆ?PLExpCutoffPSR J1509-5850?'py¹¤+ç?&Æccá_?ïþˆørÔ?&Æccá_?£nøÅÊ?Àfm4]u?îΏÉGmc?Àfm4]u?t=";"9?ŽN²ù?ïׄٙ?ŽN²ù?nç…Ñ?uX¥e"‰?ïƒúGѝ9?uX¥e"‰?,ހÜg‰?0Ú'h°Ù?ïþ2½ò?0Ú'h°Ù?Õ"/•V?¯~ª.V?w^þ‹?¯~ª.V?tRvé*Ó?jƒ¹øz ¾?ï×[9C?jƒ¹øz ¾?eD¶œ–p?[ArŒ÷Œ?ïê滋[é?[ArŒ÷ŒPSR3FGL J1509.7+5556@Võ: !Þw@Jߥ¥À9ðE;ss•À;ÉZÆõó7¿¡›÷êH7ñ@¬‹ä¥0§?ýí2?î,™¿Ó»6.\¬ ¿ß&ŸêŸ#O¿ÙÌ4mè2P¿ÏÞÇ}À AGNbll@©o5›=ÈPowerLawSBS 1508+561?ïÿ~Þ,p¡?
1"úÍã?$?Ñ¡SP?
1"úÍã?ïâ€xéÔM?}IA8Í©?m‡&©ÒÂ?}IA8Í©?ïìŽ'×ú?d5ú‰X¹Â?c:B¹ëv?d5ú‰X¹Â?ïýX*Žs÷? 0Tæ¡?5>ª|Ëù_? 0Tæ¡?ïÿÍW¾?yú?ý?Æ\*ÛC[?yú?ý?ï""£)K?­ Ísؘ?›»«šÖŽ?­ Ísؘ?ïßsl?uŒüÇβ?pFu²˜ê?uŒüÇβ?ïìÓ?ZÏÖÀ@ã?c÷â.CÄU?ZÏÖÀ@ãAGN3FGL J1509.9-2951@tù_™Ã‹@8F߸aÜÀ9›Ý÷vÅÀ;|4*©÷¶?îRJ|ÈIþ@ úô¨^@@âf'†¿é
7a|X¿ëኃ›¿áeEy±Ç¹¿ïýl*±À"AGNbcu@w®VìÔªPowerLawTXS 1507-296?ïŽtT5¡?ŠuSäj¬?Œbêðt'â?ŠuSäj¬?éϔæŠ?ÂÎDâï4<?ËøñÁ¬eØ?ÂÎDâï4<?î
òé°Í?™åµéëÈd?¯PÑfªýò?™åµéëÈd?ègé}ê?¦iæq»8Ž?Îc°Z X?¦iæq»8Ž?ïBÃáŽZ?™—ø¸@¬?—§ƒÇ]<À?™—ø¸@¬?ÓQÈÉvÅÉ?Ð|ïáÙ?æW›D?Ð|ïáÙ?éõ+øP´?´¹A¨t†m?È+QȽ/?´¹A¨t†m?Ð2KU­ Q?´1¢¬å?çæÚU)/Ø?´1¢¬åMIXED3FGL J1510.9-0542@vÿÅG@EvÖ@†À8VGõbÀ:õÇþ0òç?íÎû?0å@<k~ÿ@gŽß×@™¿àp‹Ð¦¿æm¡v»P׿æ›\2ÂZ¿è‰.NjâAGNfsrq@‹•àL'PowerLawPKS 1508-05?ïʌ}ý0î?'#ëWR}?z¹ÁE
?'#ëWR}?ìÇè%?·ÚýN5GT?»_yÀ¾Õ?·ÚýN5GT?î]‹mJÊî?š·N)f}N?ª'I*wj?š·N)f}N?é1}{€ÔÒ?¤,·ž0dô?Ë:
ü¬¹?¤,·ž0dô?íÌyjò_?²t£™a?±Ÿ<6Î.ˆ?²t£™a?Ý¥cÃ/%n?Ñ"6•W.?á-NhmI?Ñ"6•W.?èd‹†l§Y?³nÍ»£ô?ÎmÑæMb›?³nÍ»£ô?̛h«!›?­¸Êë®áÁ?èÙ%úÕ7™?­¸Êë®áÁMIXED3FGL J1511.8-0513@v)ä p¸Ð@Epà<ìÀ9F ²'/À;.¥öŸ..¿˜p'Á]O@ãRi.lÐ@EÊ`‹Ûì¿ê½€i¥h¸¿ÜüD£aÞ¿×â†G'K¿á8;ÝÉÕAGNbcu@¬C}<64PowerLawNVSS J151148-051345?ïýNÿ[Y1?1Ӓ±²ÖJ?5ˆ™ÂÑã?1Ӓ±²ÖJ?ïó'­Ûà?™üÅâ¤Ç?~&6¯A\#?™üÅâ¤Ç?ï·ðÈ2;ð?}m¥l°X?'·ð?}m¥l°X?ïë¸òò¹?JŠüs‡¤ã?dG
6––?JŠüs‡¤ã?ïõÿi4Õ}?Sle$=ò?T-Ðu
?Sle$=ò?îôŠïÞl?°þäÍa¬Ÿ? ·QµC?°þäÍa¬Ÿ?ïtTHµ.(?NP"µÀ?'uvâ{?NP"µÀ?ï4±×Ui?ˆ_ÁWp!?™iÅ}"Ó?ˆ_ÁWp!AGN3FGL J1512.2+0202@¤r¿#N@Gý}æOUÀ8zFgÃ]¸À;@¾61u?æ{S¨)Õ@ÌZÁ¶%@™ã KO	¿á½-'³N¿ã'÷­ßT¿â[eé#¿ã†Õ½à:AGNfsrq@·ydoPowerLawPKS 1509+022?ïù³SõÔ?TÌ4Y¢€l?I3õÛô/?TÌ4Y¢€l?ï"GJAl²?¤¨mÄjð?Šî-o¤Ó‰?¤¨mÄjð?ï`ëÜÌ8?–d'ãBé?"â"c	a>?–d'ãBé?îâP;E•$?†œ]Hyy?¡ÚüJÊƼ?†œ]Hyy?ïü®€ô?DØÇ1 l.?:‹AeMÞ?DØÇ1 l.?ì˥"1?Â⎺ed?¹¢Ñë^w?Â⎺ed?ïÈöSƒá?˜DÄʽÜ?œfá,ø}ø?˜DÄʽÜ?è‹ÍGéE ?¶àȹ4?ÍÐÊàZë€?¶àȹ4AGN3FGL J1512.2-2255@uH^`=Wy@=xœ \–ÚÀ9â¾÷!À;d-–;@H?«†9¸¯õ¬@
®µëÓ?þôÿÆÊ)?ïËuȕ@Ö¿åïÿµ_ü¿Õ"'
»¿Û&ón¢AGNbcu@©í›"Ðå`PowerLaw1RXS J151213.1-225515?ïúcÕ"Âß?NWUò\ó?Fpªí·Í?NWUò\ó?ïÃHÌøk·?˜ùXŒ3*?~[™ž—W?˜ùXŒ3*?ï¸g9—rÅ?~ËDÊÿÔ÷?æ1'ê¬?~ËDÊÿÔ÷?ï炀ÖÝ¥?Sz-ͺ©?h}"C"Ÿ?Sz-ͺ©?ïõ‹Í©¸?SX\Ì­lÞ?Tèe,F.^?SX\Ì­lÞ?îÏ8ßîŠ?±G4Ä@/?£~ñ%0a?±G4Ä@/?ï•:)F M?‹5Àï-{·?Š±u¤	´?‹5Àï-{·?ïV'"
9?†_ÿJ÷•»?•;½~XÔ?†_ÿJ÷•»AGN3FGL J1512.3+8005@\ýÃ?…Q
@A†ªšêÒÀ:›Ò‰¥/ÐÀ<*y®AÇK¿'&†ç
@Œj€ý@ˆ@ò`…%ï¿ë¥ìp¿äø,"¿ã'l"	ì¿ã3-ÇcZAGNbcu@‰œ¯hیPowerLaw1RXS J151026.3+795946?ïô§èos3?a"mÛzº†?V°/kQ)?a"mÛzº†?ïÚ¤$ѵY?ƒši´Þ¹?r­í Ož?ƒši´Þ¹?ï3.1&ú§?šWÑ8œs?™š9ސG?šWÑ8œs?ïöÿ‹ïj?7ÿYÈP»?RçŸù'x?7ÿYÈP»?ïõEß)¾?bљö˜Æ‰?UtB-µ7Š?bљö˜Æ‰?﬛ÿÐZ?ªÙÁÍ¡P?žŠl†å,­?ªÙÁÍ¡P?î¬#S¹‡î?¢Cn@"½Z?¥=ÊÀþ'?¢Cn@"½Z?ÁþÆ"?{Gã "Ã¥?ˆO'|ƒx?{Gã "Ã¥AGN3FGL J1512.8-0906@uôŸ`—Ì@D?ßéàÀ5nV·œ¹àÀ:¬²{ï@_"͊aî@"$åg£R@" ¿M¿âR´ü²©Ç¿æPH	"
@¿æ—/˜¿è4š7½ö4AGNFSRQ@{Ó -à
LogParabolaPKS 1510-08?ïÌ\Í5?–Ë«Þfû?yÿR5Íc?–Ë«Þfû?ïؓV"eI?'
cáôÍ­?s¶TÔ°Sj?'
cáôÍ­?êÅb\|€?°…*]tðÛ?Äêvî
ÿ?°…*]tðÛ?ïÿè-®íq>á'²Ö)>çÒfŠ[ d>á'²Ö)?ï-O_tëË?¢B|ëý®[?šVTŽ?¢B|ëý®[?îï‰}ö-¢?³30¼²å?¡h-‰ç?³30¼²å?ìµRº·÷S?ªÄÍ$æˆC?ºUj*@Ej?ªÄÍ$æˆC?ïÿøOK[>ÕÙUœ["b>ÎÃŒF	>ÕÙUœ["bAGN3FGL J1513.1-1014@uåóà7Ý@CžŠÿ¢âîÀ91#ã4À:¨Â<Pg¿Ý¤}6Ñ<7@.ëBƒ³(@ƒ@;ÚL¿çÄëçf£o¿ê‡a(¿åõ—1´6¿ïý°<÷'AGNfsrq@‡Îp:ûPowerLawPKS 1511-100?è›`?ÌÀ°I^mÊ?Ïé"ó΀?ÌÀ°I^mÊ?ïÐÄ–?$œé´?w÷øΡ!?$œé´?çxwmÛâ?±ú~BÈsï?Ñç$H<?±ú~BÈsï?ïåM©¤»?U—ÊîE	?j²à#
€?U—ÊîE	?꾧GN•‡?Ĝ6íQýy?ÅbâÅ©å?Ĝ6íQýy?îÏ€Jñž?¯ÐazP?£·ø½1?¯ÐazP?èÐÞ¡­Ý?³^}žBI?Ï༅yHŽ?³^}žBI?înó}!?¡‡íýL†?¯ImX'õ?¡‡íýL†AGN3FGL J1513.4-2549@u-ÿ¼ä!@:÷_f—åÀ9®P(6ïÀ;¦¨ñü1>?ùX,)(ÃC@GõM?ôò¬O©¶r?ÎÕÐxö-¿ÞB1õÁÛ¿éÝk±åüÛ¿éVcCÇ*!PSRpsr@'Ä"t¼LogParabolaPSR J1513-25?Ìäãoüg?ÉYÆ^¸`ô?èÆøG$æ?ÉYÆ^¸`ô?Ñä\ýBF³?ɝSâë?ç
с^ܧ?ɝSâë?áŒo'‰?·K¨s0Œ?ÝÎçé!°ï?·K¨s0Œ?֍†=Œ?°PUb?ä¹<ð~á:?°PUb?¦Ê‡_Eºé?²¶Iµ'U?î"WŠbÁ?²¶Iµ'U?®LS?Œ¿?³ÏäB—ü¢?î:γô?³ÏäB—ü¢?Ð7Î'ë¬a?¾SWjõí-?çäì
)Ð?¾SWjõí-?¤FÐCÛ¿1?'eHB߯›?ûù=Í?'eHB߯›MIXED3FGL J1513.5-3233@têµ_þmY@5këß·‹À8úaPÀ;[ƒäün{?ò¬»y"@ÃæÄŗN@¹áÀ¤ËQ¿ßn [·ƒ1¿æ:À&4Œ¿æ×G<Tš¿èœÉ@j:AGNfsrq@ˆ×hr°!PowerLawPKS 1510-324?ïúp4#%Ó?Dm`Ö‡?F?/?_u?Dm`Ö‡?ïű§¤Á?Œ¬XÞÊmz?}','1?Œ¬XÞÊmz?'‰»ç?…{cl™­Ò?Ž\›«Ov ?…{cl™­Ò?ïê'Щ{?J2îE4ä?epØ?Ô¤°?J2îE4ä?ï÷4'áÈ?Tù­xò Ä?Q—°'¶ ˆ?Tù­xò Ä?î™?b|³?¼^¯d¶?¦l	Õ¡±?¼^¯d¶?îÒöN‰¦?˜ówj÷n?¢ÐŸí«Ÿ?˜ówj÷n?ï¾.yîŒ?rd-­áoß?€ta"ƒ#ó?rd-­áoßAGN3FGL J1514.1+2940@GÒtw@MQ™?׆dÀ:/àÇU"‡À;­ä9ÐÜ&¿Ý"žfC<&@w€*@Þ§ªÿ¿éªASv8…¿ìLû^ÿغ±Úá–¿æ3ɖ¿þAGNfsrq@}«¾ ºKPowerLawMG2 J151421+2930?ïÿ»*Ò«M?
p™.?5C¯*#?
p™.?ïދ°Å&³?ŽSQ‹¸ÛS?pº'{Àzå?ŽSQ‹¸ÛS?ïÖÉÑMm¥?|å«ÂóN|?t›JÚÑÁ?|å«ÂóN|?ïýÝܼ ?j<2ùH?1ó÷Òa?j<2ùH?ïÿѓÓSq>ÿŶ>…ö{>÷6È~^ƒ>ÿŶ>…ö{?ïií³™—?œ#©AF52?'ÌBN´7
?œ#©AF52?ïºßƾY±?~ÓD–ÖZ?HFÊ«¿?~ÓD–ÖZ?ïí`øH?\/M]qnY?b€žçxk?\/M]qnYAGN3FGL J1514.2-4947@tS°€0<@6™_·ö|À7ßÇËÜÀ:à)q'@å[½•ø@±aˆŸ?üûòª,¿ÓÛ'~Z¿×Š
oª1í¿á"Á0¿îö¿ëhdj/@,PSRPSR@˜Gâ'@¸PLExpCutoffPSR J1514-4946?Lâp6ù`?WZÝú¥*Ð?ïøÇcΨç?WZÝú¥*Ð? c9À}ú?·}ˆvC™¬?îþ9Ìu?·}ˆvC™¬?¹n³¹Ù¿Ÿ?©ñIM¹·À?ìÒ)ˆî\?©ñIM¹·À?€žýéõ±ƒ?fˆÒõwe8?dI
ò?fˆÒõwe8?Y >܊?SRê·²?ïó/öEt²?SRê·²?'F$nͧ¹?«€KKÐ/z?ïuÎÜ¥¢?«€KKÐ/z?Œ³MtÒåÁ?ˆGQ?'$%?ï2Éçü9?ˆGQ?'$%?M¬\Wj/?A¬Ižù?ïø"èɜ[?A¬IžùPSR3FGL J1514.5-4750@tdñà'Œ7@ Þ#ê¬À8ÅÅ.î*À;-R,¾?ãË4ôJât@àjR¯$p@£q ?[¿åݕH•ßÀ¿ä­8Íw¿àõ6â%Šº¿ëF'9LAGNfsrq@Ç‰"SPowerLawPMN J1514-4748?ïïjëuR?^ÇC"`æ?`•Ç[Ír?^ÇC"`æ?ï'n-É֒?•;Æu\ÝØ?dtŠ¿'?•;Æu\ÝØ?ï@?Ïèz?•«Z,?ŸWø	rŒ¾?•«Z,?ïqDEÌ?nûP¿õF¾?'×}rë?nûP¿õF¾?ïÒëæ 8?v^Åý·¤?vŠïã¹_?v^Åý·¤?ëóö Ð||?Áÿ'C>»?À0'|¾?Áÿ'C>»?íp©¶GO?¤»Ú–vêç?·,z²»¹?¤»Ú–vêç?ìYµ4P?¢lv¡¢ª?½2Sö]{?¢lv¡¢ªAGN3FGL J1514.8+4446@R‹UŸÚ%{@L7W`9%»À9J\OÝÀ;ÊÅ-œ}?íúgPàÜé@ÐîÕÒ°@¶G_eY¿àa·ã[¯~¿å"ÐèBþ¿å™‡¿Á¿ëU'Ö¢}]AGNfsrq@‰ˆLáłVPowerLawNVSS J151436+445003?ï³@e~h?'‹—Õt"1?ƒ8oÕrZ2?'‹—Õt"1?ä?«'ýhç?¤g¿¹¶<	?«'ýhç?ïtó¼!0?…•3¥Á=?'aˆg4p	?…•3¥Á=?ëÀÿ*ܼ?—Ñ¡~݄?ÀýÀT?—Ñ¡~݄?íU­†‰?µÊeæÐ?µR"Ð˳?µÊeæÐ?ç)áQ'îK?ÎAŠìÿ6?Ѭ=\ú#j?ÎAŠìÿ6?è®´~ªÞn?¸ÛÃ)/Û,?ÍE.T†H?¸ÛÃ)/Û,?Ù[õ
Ïv?³Á³6§?ãR8yE?³Á³6§MIXED3FGL J1514.8-3623@tÊ # –@2Ù_'F—À9ë>nИ3À;‹<R–¥É?ê©idð@oèך[6@=¸¸ÇÝ?âºT£‹¿ç,.õ¿gè¿ælõùÕ¿í/_[&¹ AGNbcu@Ž:F§ï²PowerLawPMN J1514-3617?çüž\³?ɪ‹,Lâ?ÐÄÃF™Ë?ɪ‹,Lâ?ì°dî…óä?¸Z—8žà‰?º|؋Ð`ß?¸Z—8žà‰?ê¶"øÔ?¬¡Àþ'?Å'ñ°Ü®?¬¡Àþ'?êq±Ç†? "@\Šœ0?Æ9½8ã©ç? "@\Šœ0?âȳi¼K?Ïy˱LqP?Ún™Ã,‡j?Ïy˱LqP?àw賡ò?ÑfÙö"}ü?ßù.˜¼?ÑfÙö"}ü?㴈ldq?½Œñž1?ؖï'7ñ?½Œñž1?Ô$əͭ.?°sð07?åí›3)i?°sð07MIXED3FGL J1516.7+3648@M×­€k`@Lô¯ÀL‹ÊÀ:s[Ÿc6À<
ÅÓ´G›?ã'ã鸯£@Ö;‹qc@שjÄD¿Ø‰Ö«Ñ]3¿â­vû¿åuÒùüI¬¿ïþ;g4A¦AGNbll@"Loƒ{J#PowerLawMG2 J151646+3650?ï*©ˆé¸?µÖW±+?š¼êÎâÉ?µÖW±+?ïdzK$K?†Ðe¸µvl?|&Zsp:}?†Ðe¸µvl?î1¾ðAW?š•û‰nk?¬ä ?š•û‰nk?ï& ^ƒO?{!æY»³?›+ô5ؐ6?{!æY»³?ï7ǵ"T"?žÔ³Ic¹?™	K½Ÿ‡?žÔ³Ic¹?îž)1»?³Ô9ø{$¯?¯¶mUS?³Ô9ø{$¯?í›32î?¥!ãeѧ8?·¿K%øu
?¥!ãeѧ8?é‰ØŒQ:8?²˜Þ6?É؝λ ?²˜Þ6AGN3FGL J1516.9+1926@;՘Ÿž–Y@KëÀ·pDÀ9Öï
wÀ;µ"'±ÈÀ¶:¯³â@ül¦œau@#ìÀ24±¿ænž¯¿1¿êæíZ¿çû÷–5GF¿ÜÛý`':œAGNbll@zá2µ_PowerLawPKS 1514+197?ïþØ°…ÄP?"ç!Üy‹-?"tö0zÜ?"ç!Üy‹-?ïá=ÙÄæ?‹;ž@ç4?nÂ&p)h?‹;ž@ç4?ï¿-Ü(œ?x)sÓE:?€4¾¼+?x)sÓE:?ïÿûLUÝÇ>»4#@Ñ>ÂÎ'¦eX>»4#@Ñ?ïýF§%À¦?;_âèîç?5ÊÆDB?;_âèîç?ïe_"ØК?œ¶@Åø/B?"Tž´Ò?œ¶@Åø/B?ïL¬lÌ?ltZ`lÔ?–jrzöà)?ltZ`lÔ?ïÿ7$¦ÊÒ?âH|ÕÍ1?j÷–¡R?âH|ÕÍ1AGN3FGL J1517.6+6524@YÛa»û@F³'Àa"À9OŽuy)À;L	ÃÎ!¿õ`‡·™ß»@sIcKSæ?üƒ—
&Y?{­5F¢•…¿ã-dÃ2¿Óƒª3ða¿Â~	ZÇ¡ÀAGNbll@«‰c{J#:PowerLaw1H 1515+660?ïýÿñµÝ?)¿ÖBq?08@ÖºW?)¿ÖBq?ïÝÃdÄ$Þ?‡Oõ:óÿ"?qMí'=?‡Oõ:óÿ"?ïކ§¾9P?põ'‹×?p¼¬
åØ&?põ'‹×?ïÿöGÿ>ÌŒrâ">ÓqU í©>ÌŒrâ"?ïýyØ´¶?1%o›ÿ}¯?41<﯐?1%o›ÿ}¯?ï@5£¬‹?ªª2'%;?—ùKò š?ªª2'%;?ïËCRe'¢?€88ë€Úm?z^VîhnÏ?€88ë€Úm?ïÿ"Q3¬Þ?:ÃÉæŒë?+¸0Ã}?:ÃÉæŒëAGN3FGL J1517.6-2422@uJÑ"Dž@;"§@KIªÀ7es!_ÌÀ:ÔÖ-žž¼?Õû¶_"$m@eÓ|"P/@å±_³ï±¿ã#oڔœÁ¿á¨ãîžÑ¿à
¯€ƒ"¿æ"YO@tAGNbll@8FÜ]PowerLawAP Librae?ïôUìŠq!?YZ2±o,•?WT&û›Ý?YZ2±o,•?ï¦øm˛±?Œw*ÏyŠ?†A䉩wã?Œw*ÏyŠ?îÈÝ1§v?£ü֒¹Ïœ?¯£r,刨?£ü֒¹Ïœ?îÙ¦ÏãÂ?Žnôéò-¢?¢e"ÏãÙ?Žnôéò-¢?𢡊-?…ð¹Äð?…4Ì·êm?…ð¹Äð?ì*,è	®?Â{)'Qäµ?¾®Ÿ˜¿²'?Â{)'Qäµ?íØMàøA´?¤?[jÌá÷?±=ùõÀZ?¤?[jÌá÷?æB¶=Nü?½Gé"ÃÏM?Óz"Í…b?½Gé"ÃÏMAGN3FGL J1518.0-2732@u*­ ‹]@8ùx¿.~™À8šRÙÀ;$C£Ã¿¿À€+q'Æ@"ÂLÁ#Ì@‹Ÿ°ßÜ¿ÞcS÷ÎÙ¿äâ=X¿Î{¿àÃQ,(¹¿â>*þ0rAGNbcu@š†³3333PowerLawTXS 1515-273?ïÿ¥d~ç>üÈÌËå¼Õ?¦ÑrUóç>üÈÌËå¼Õ?ïϖÿi	â?‹PÂo]:?x4€6Ýfí?‹PÂo]:?ïὨJ??mï›ëð´Í?nBW‰Åä@?mï›ëð´Í?ïû&òˆE?,æ=ÐB$?Cd5íÖ8?,æ=ÐB$?ïÿqõ2>
?èËa?ÁYË$?èËa?ï	š!n?°àL¦¡¿Ù?Ÿü>ËM?°àL¦¡¿Ù?ïÓ¹¾°²î?~ªª¤^
?v# ŒÙ"÷?~ªª¤^
?ïÕ*Ô6oö?fÉðýH«?uj•Û)?fÉðýH«AGN3FGL J1520.3+4209@QG¿@OÂ@L_×ÖìÀ9³—>u‡À;ÝWªå?ì/xB~L.@5¬µ*D@ýXÌ¿àv›"_aÔ¿è¿\"ÞýZ¿çCvý<½¿ìPa¼Þm3AGNfsrq@"Ð}!ÿ.IPowerLawB3 1518+423?ïý6þ{y?0TOZfPš?6OîD¸_?0TOZfPš?ﺋF`?‹ë¬Ü£vÁ?]?ß³–/?‹ë¬Ü£vÁ?ï€Å²H´q?'%€í¤&q?Î"`sÈ?'%€í¤&q?îÉnxÐï?(¦53—?£n™rñ?(¦53—?ïýKXª!b?3¸â{éÅ?5¥8ڐ•ä?3¸â{éÅ?íÃb`uW?µ5šékb?±äìþ®aÌ?µ5šékb?ï A'<–ð?"U¡Ôó%?›÷ϻܽð?"U¡Ôó%?è	ävÝ?²8áYô?ÏÏØoî$‹?²8áYôAGN3FGL J1520.8-0348@vaä?åÉ@E@Ì?ß À8ñzbœ­JÀ;B…¶Æ?ìù×	Å.P@þC"¨"Ý?ýXà¨Ì½?æ6Ãì±ø¿Ø¼c,9ͿΕE=-­¿à$¡Vk5rAGNbll@©/˟U›=PowerLawNVSS J152048-034850?ïÚás´þ?r¦ÁëX?rF%F•?r¦ÁëX?ïbè¡$ä?˜\UøL?"½¢ïJÿl?˜\UøL?ïjÿ?IB?Š¹ð'~ç?' $>A½?Š¹ð'~ç?î'G:.؎?Q™«¤?­‹ŒZ~Â!?Q™«¤?ïµ9ƒaýT?€®»7£®9?'±Ÿ0o§?€®»7£®9?ë¿U.Ê]?ÄÞn_ÚE?Ñ«D֎?ÄÞn_ÚE?ïUõw]Q?—ÞËÑûŽ?ŸµAM¤¹ã?—ÞËÑûŽ?é'%ÄñÈ?°1¯ÕHÐ?Ëÿchì8ß?°1¯ÕHÐAGN3FGL J1521.1+5543@V‰?ßéà@Id›`C6¶À:{7ýJCÀ<#ǃ·°?á&D"He¹@
È—ý¸'@]+éTm¿ìQßÅC'¿Ö.î"Fe¿å=äð¥¿Ô?Áœ"[AGNbll@œçÍquŽPowerLawSDSS J152034.98+554256.9?ïøïÔÓpD?]/m'Ó»?L@­3üüÞ?]/m'Ó»?ïΖ×P?‡ö'Ë1Ro?x´"QÈ(?‡ö'Ë1Ro?ï¡ßûË	v?"Àà¹'?‡ˆ	Ο?"Àà¹'?ï›I'³«?rÞ"Æ
´7?‰-ŸEa%b?rÞ"Æ
´7?ï­hxºPô?ŒPç0ø±²?"¥áÔÛ^í?ŒPç0ø±²?íæZ"[?·ögßd{?°Í/:ñ'ª?·ögßd{?ïðΒR?•ÛŽNj?Ÿ¿ÁéQ°?•ÛŽNj?ëOÈõI:(?µiÉ9bâ?ÂÀÜ*Û`?µiÉ9bâAGN3FGL J1521.8+4340@QæïÝëÙ@KÉN ƒyÀ:$ìH"ÉÀ;×#{/K?×ÜŒ{›@u^>#Ò@Ú÷àvͽ¿æß+‹7ðÌ¿ëš{Òðd¿ç^õ }ùֿڕTV0ŸAGNfsrq@…ÂpØDÐPowerLawB3 1520+437?ïÿã­~'>î·eØÍØ>ìR¹1Ñr,>î·eØÍØ?ïßÃO~ ?~¼"Òçµ?pX+¢\—?~¼"Òçµ?ïÞö®Ù­í?p¯Ð²p?p"¨—H'€?p¯Ð²p?ïô'†iå?@/Õä‡h?VÜóXû5j?@/Õä‡h?ïÿӁ5¹d>ø"+o@>ö?K¢Ø>ø"+o@?ïe
×ۅ?£/'
$d?s^£LÁg?£/'
$d?ï³@:Çjý?v7X2?ƒ/ñUx¼?v7X2?'À%c?\pÂØ{°?Œ[VÕß!?\pÂØ{°AGN3FGL J1521.9-5736@t VàL'¿Ûd _þº¨À7d˜$ qÀ:D˜n#Ê@d—.Z[@Xç×Nl@=Ã/@¿Ï•¦'Gã¿áǼ¸é§4¿è}M÷7b ¿í ÞW
ØÜPSRPSR@ŠÚh	ԕPLExpCutoffLAT PSR J1522-5734?%'ïW™u"?$®{FÌ&/?ïþ¦áM.Ô?$®{FÌ&/?§c¿ØrV?Ãk¾aqo?î‰Ä½ŽZ?Ãk¾aqo?ƒÙ2?Ô'?‰×œš‰Z?ﰛ6ãÓ
?‰×œš‰Z?ÃGsú&6?tªÅÑ?ïyåÄ6ó?tªÅÑ?+aÙgìçý?#5ð¿Zz?ïþIâL:ì?#5ð¿Zz?‡°ÐizÈ?¨†©8.Uå?ï¡<¾LVp?¨†©8.Uå?uÍD"?hÞd_c?ïÕÐe¢`?hÞd_c?_Ô'ãŒÊ?RŸÞrk?ïðëéar?RŸÞrkPSR3FGL J1522.1+3144@IÓßæ…@L'ßý`éÀ6FchÀ:£ÓöeM?û¨w³?Ýæ@…éµí¸@~ÓnQ—L¿âN¬Œv¬–¿åʍ¿	¯p¿æ]J "'¿èÏÅÇíAGNfsrq@sc}ŸÓo~LogParabolaB2 1520+31?ïõÔ±ûˆ?[–»Ô9 ?TWܬ‡º?[–»Ô9 ?ïÖ{©»ó?'Pɼº•?tÂ+·ªò?'Pɼº•?ï,±é"ú@?"mu8@B?šiẦ¸?"mu8@B?ïù¯Påö"?:ÚsF°»?IB¼uä'?:ÚsF°»?ïå~£(?làBǏ
?jðWbxT?làBǏ
?ïUE6•é6?¦ÈYËxcê?•WY0²u??¦ÈYËxcê?îÉä$#à ?š°üÏ®Zo?£a½¹xK?š°üÏ®Zo?ïøã: ª?L^:‰òê9?LsâçÜ#e?L^:‰òê9AGN3FGL J1522.6-2730@u9\_|gZ@8f6îÍ©À8$l"}ÐæÀ;žîm0…?ò³üY,l@Öâ'ܼ@"à)ËÖ¿Ùkë[-M@¿ã^¢;˜vH¿àTË«±ì¿æ´œ.ÊBÚAGNbll@–9y#¢œxPowerLawPKS 1519-273?ïþŸÁžy?$"þ­õ?&ò=7	?$"þ­õ?︠í˜@Ë?Ž"Z÷X¢À?×ę?á%?Ž"Z÷X¢À?E†Ù?ƒ­!ºÓŽ¨?‡X˜®žI¾?ƒ­!ºÓŽ¨?ïw—»X?g¾
ê»?ˆ¢H_þ?g¾
ê»?ïý…û"Dý?2ó¸°¹Ì?3Ð%
'ö1?2ó¸°¹Ì?î|p¼*¾?´¡tîå1?¨8ô<x7f?´¡tîå1?ïf)	.µ?'påŠ!Æ=?":Þá÷P?'påŠ!Æ=?îÆ-²'
?>YUQƒ:?£.4×ß6?>YUQƒ:AGN3FGL J1525.2-5905@t8–ž=¿þm)Tc¯À8äç
À²ãÀ:QÎ2þZ?Õ®ËÄu@
½U5'@JÛ`cm
¿æHP¯×ï¿æ©³ÍÍRÚ¿ç
'¿ç-BÀÜ1AGNbcu@'y¼j~ùÛPowerLawPMN J1524-5903?ߤ4iág†?ÕÏYÀ¡×g?à-åËL=?ÕÏYÀ¡×g?ï[<bö‰#?žÈÞÑh/B?"˜s¦VE¦?žÈÞÑh/B?å<}‰ÃŽ?»Á©ÃˆUz?Õù‡ìxå?»Á©ÃˆUz?ïºßqêþç?b
ìe–ú,?H#‡P
>?b
ìe–ú,?Ô¿†Í(>?Ó<7½'?å <™kÿá?Ó<7½'?ê€H©€Ü?ǁte=؏?ÇÝþÝYü?ǁte=؏?ã7X‹ Hå?½kµßå>?ّNé¿n7?½kµßå>?í¥›Wã?›ƒ–ßWw?²Ó'ÆøµN?›ƒ–ßWwMIXED3FGL J1531.0+5737@VæPß´0@HS?Ýe¡À:y¿ß~€À<¥šXÜ:?âÛ$»#ù@q|ï>çœ@%±ÀVò«¿çíÐ
¿áœF7¥f_¿åRkuwƒù¿µÀ½mÍAGNbll@"Y"Ý—öPowerLaw87GB 152947.5+574636?ïþvô0Ç|?/p¢ˆ¦©§?(¹9'ý5?/p¢ˆ¦©§?ïÝпds?€jUKpr­?qp—'{?€jUKpr­?ï¼­'·ç§?n֔ý½?€Ô›˜5b+?n֔ý½?ïèŽMwç?SÞ"– ?gq²®î1x?SÞ"– ?ïòÙåÎ+?bëܘ­ò}?ZL6"˜ó?bëܘ­ò}?îů
*a?³aq±÷s?£¥`Ƀ?³aq±÷s?îÁ}œå1?ž›@r<Ü ?£è/w
"ì?ž›@r<Ü ?ï	¨tË%z?•ûÚ	(ü+?žÊñmzˆ±?•ûÚ	(ü+AGN3FGL J1531.8+4704@SýÀ?`@Jr¢ŸÒ˜¿À: NRsj[À<ò¢Ik"?¡øsìý=@
ð*IÏ,@†Aßsm‹¿ëÜõB¦‡ƒ¿Üò4@à¿æI§­Û¿Ø
«(t‹AGNbll@"i
ÀƒoPowerLaw1RXS J153148.8+465912?ïó¦	-j
?i~ì÷
ø?X³í¸i»H?i~ì÷
ø?ïۚÖÔÛ?}ÏÀF}z?r2øzxŠ·?}ÏÀF}z?ï.®;€ù?" Ó/ù~?š<ê6ØØ?" Ó/ù~?ïìõ¨}Ö?P ´*ƒ?c
W¦hâ¨?P ´*ƒ?î#Ð~!û?¸]¡øú'?­Âø!_,S?¸]¡øú'?îµv'TG?µ.~7{\ç?¤¨Ž2íš?µ.~7{\ç?ìÅ õ³?´ö{&Nä¹?¿<ÖøRj?´ö{&Nä¹?îÄxnÀkÚ?š¡:G°Šû?£¸y[^?š¡:G°ŠûAGN3FGL J1532.0+3018@Gì:?–îÄ@KhZ&–mÀ:!=ÍÀè"À;´:ƕ?Õe™W)‡Ž@[¦nê?ü>AFœG?ï÷aÐu‡¿Üh‡Š…¿ÑY¤£°@G¿× ‹ŸÊ¤îAGNbll@±|öÈ´9XPowerLawRX J1531.9+3016?ïþžïüü?'ѝöĈ?&
³ç?'ѝöĈ?ïß7qög?wj¯N^?pdFüÀ¼½?wj¯N^?ïÎ;l'¥_?wcî¤S?xâI¨>ôÅ?wcî¤S?ï坷ý!?T/@Ž&P!?jbî+&'g?T/@Ž&P!?ïù':,v¬?K9—öoܹ?I÷çúv?K9—öoܹ?ï!»ûÝö/?¥·,OßÔK?›È€"A:)?¥·,OßÔK?Q
tï?†äóËnqÛ?‰Ýk²SðZ?†äóËnqÛ?ï€lU­u]?…eèg2N?äê˜D¡?…eèg2NAGN3FGL J1532.7-1319@vHÿ¸²d@@Ü
`:Ó;À7Ý[+J1À:êè'œ&<?èݯr–Aî@@‹Emó@À…Ü.?¿×!R¦ý¦¿á"­Þ8ô­¿ãÄUã4¿ßó¶ËهÆAGNbcu@'œÄg8~PowerLawTXS 1530-131?ïÿ¨"ÿÉ?¸àät?ÚýÛ§Fp?¸àät?ïÕ«,>!?"úÿäFþü?ur*Œ=?"úÿäFþü?ïzAû€œü?¤ª¢^ê?·À–˘v?¤ª¢^ê?ïÿû¤ëK,>µö=ËHŠ>ÁlPþ¨~}>µö=ËHŠ?ïÿ\ù̓M?±;%$?`Ëò%|Ø?±;%$?îö°¬ÁЬ?±örûò•Ž? "õ7R'B?±örûò•Ž?ï±:†IìÄ?ˆýå3ûùï?ƒ±^jÅñ?ˆýå3ûùï?ïÿûÏÞhð>Å©¥Nž¨¨>À¿î£ƒxB>Å©¥Nž¨¨AGN3FGL J1533.2+1852@=)@ªÀ3@Jÿ—$tÀ:0;eÀ;¹ãÕ'b¿ãùB¦Ì;@
ŏb^?þOà2ZE¿é†lêJ¿åÞŸ¦Eq?½‰Jl	éc¿Ûù˜áýzXAGNbll@­å‡E8ï5PowerLawRX J1533.1+1854?ïÿ'Ø- o?éT±
œì?Z¡;?éT±
œì?ïæå!'[º?sî¥hÈ~ÿ?iÞ;«Åö?sî¥hÈ~ÿ?ïãúÊGG£?hñx'ÚÞ?l5ʖT~?hñx'ÚÞ?ïÿÐ-!?
{'=d©C?ÜÂfb?
{'=d©C?ïÿEÙS?‡EOŸí?—DVç?‡EOŸí?ïOçâZ†?£5…žºì?–ã´¯9?£5…žºì?ï˖=2H?{ƒÎÉÊÚ?z4áfp?{ƒÎÉÊÚ?ïùÐ3'1N?F¸4m¹1B?H¿0ÀðbÊ?F¸4m¹1BAGN3FGL J1533.5+3416@K_{Ÿ³@KU@ÿ¤nÀ:lÃÕ­FÀ;ÕòJ4×x¿Òɐjc@¸©Ý3¢D?ý«:ÞÎ,¿ãSÛýÊÏ$¿ç$8vi¿°T÷†½R¿ànG˓RAGNbll@©#a$Ý/PowerLawRX J1533.3+3416?ïÿ`Ú"?®Ï?þÉ?íýņb•?®Ï?þÉ?ïÞØÁ³Ð8?ŽN2\ƒ?p"Ÿ&ÇÐ?ŽN2\ƒ?ïà©]±áå?g^¿õï?oV¢%›z?g^¿õï?ïú
Ò
v?5Ü´óXVÕ?GÇÓñ੸?5Ü´óXVÕ?ïþwýñ«?(oE)[ÓÖ?(€!®Uø¥?(oE)[ÓÖ?ï&`T²"?£wäž<Ðó?›3õbޕ¤?£wäž<Ðó?ï¶j`N§á?€E‹éwr?'egäÆã²?€E‹éwr?ïÏ	¤)ќ?tëgÖt´'?x{-æG¾?tëgÖt´'AGN3FGL J1534.4+5323@U`7ßÕ¾
@IE`\a*À:׺nü7À<!x#'L¿Ý•VpqyŒ@uuœ9\?ÿZÞ°t|¿í9"ZÌf¿­š"i´¿ÐIÀ	è-ž¿ãŽ…ÎØâýAGNbll@¦%ðå`A‰PowerLaw1ES 1533+535?ïþF÷'¥Y?2£ïªŒÖ?+‹lۉ.?2£ïªŒÖ?ïօ40?‰Ék	?t½eÒõâA?‰Ék	?ï»Ýה¯ƒ?€¯X> Ê??Š)ògE?€¯X> Ê??ïøìºAɓ?8§iøF[?LM££eM?8§iøF[?ïöd±Ë?T¥¦Ù TÎ?S7Ô&66O?T¥¦Ù TÎ?ï[Ó»S~?«CAÖ¨?œ"…tÈA?«CAÖ¨?ïk<ŸT?'DëžGt?'ú#ãƒ?'DëžGt?ï¬*·öÌ?€	£šáܖ?"õRF¼Õ?€	£šáܖAGN3FGL J1534.5+0128@´‡ßÝË£@E¢¿ÖDEÀ9r´€ÈÀ;9oV•¿÷RH¿·e‡@ä8¤6V@:Ä@]׿çõ*åd{Þ¿ê%…sÌοã2¶¨ö¿ïÿÂáo#ØAGNfsrq@xòpÃL‹PowerLawPKS 1532+01?ïÿ[hZ?ìzóáw?'êhþ­?ìzóáw?ïׄš?B?…ܵð^Ä©?t=²ÙºU?…ܵð^Ä©?ï`¿Xc?Ž?R?"èô%Mº?Ž?R?ïÿêh`ˆù>܏oV¥Ó<>å—Øüçý>܏oV¥Ó<?ïÿÅÔFO?y'ÿžþ>ýÉä"9À?y'ÿžþ?îö·WÞ?²À'#§? "ŽKj‰!?²À'#§?ï…öÞE#?{!«Ãµ?Ž'xV-'8?{!«Ãµ?ïþÎáÈÌ?"ٗú,oô?#ÎHiO?"ٗú,oôAGN3FGL J1535.0+3721@N: þ¡@K.ßç[ÄÀ:kc%iFÀ;èa'ÑÖø¿×IñàO@UáŒR3@é¾ RÔ?¦:A^2ÿö¿ä0+Y¨›s¿è¨ærT+?°+n"ï¼AGNbll@™"0¸»PowerLawRGB J1534+372?ïóx0¤sÎ?ŠDm=&Cd?YŸb²?ŠDm=&Cd?ïÝéÀ"š_?ƒÔ2—?qÑÖÊ?ƒÔ2—?î"H?",NŠK Ñ?ºZ‹:&?",NŠK Ñ?ïþPd5M"?@èÇ?*ù½‡"?@èÇ?ïô^ôظ?[¿gDl?WB¸l°:?[¿gDl?ï9"Ǒ_Ê? ØÓöt¬s?˜Û§¬œ¸? ØÓöt¬s?íÁ2{c‰Î?¨òp	"Iž?±öl&›‹?¨òp	"Iž?ï٘ä#;Õ?r"Dk˜î?s3êBF?r"Dk˜îAGN3FGL J1535.7+3920@O«"?½…1@Jó®ñðÀ:§ouÙ ñÀ<bfýe?Ý©¥wÀ£@@d•Xí,@Ë.@/E?ïþ¼I$"½¿Ý³"ê÷Á¿ç>Ԁd-@¿ßÓÜW>ÅAGNbll@!¡ÊÀƒPowerLawRX J1535.4+3922?ïNÑìK?Á"÷,‹"
?–%Þ¾Ñ=?Á"÷,‹"
?ïӖ~öÄÝ?€.ÂÇK•?v4Àˆ
-¥?€.ÂÇK•?ïu^ÏÄ?•ÉÛDŸ?œñ_жk€?•ÉÛDŸ?ï–]N‡?s"­(›&?Šh¬ZÊ"?s"­(›&?¨gV•?®Išé$ò(?ŒÚUØkêÉ?®Išé$ò(?î"ÇÇ̪5?°†_ÔF«Å?¦³ƒ…ɳ?°†_ÔF«Å?ìÛ;¾$Æç?±´pú'Ê?¹&"
ýáÆ?±´pú'Ê?ì }m¶^C?±ûȇ»?¾ü'M
ê?±ûȇ»AGN3FGL J1536.3-4949@tƒ!_Ìr@ Þý';À7)&p­À:"&êþ@&»¶Où@y6R!Šê?ù×2
ï+ò¿Ù+¹öËпÜh‡#±q8¿àKª7m÷Í¿é=ORòPSRpsr@NJ	ÞLogParabolaPSR J1536-4948?©n'joR?­­½aå?îiïۚ›?­­½aå?¤É?¨Ñ3Ô?¿2<{'á?î³l·¤ò?¿2<{'á?ÚFÜèù©$?´_6pT
?âܑ‹ƒ+n?´_6pT
? t›z6«?"öµG'È?îø¶öVU?"öµG'È?§P®(¿3?¨Ÿ§Ï¸«?îŠþEb,<?¨Ÿ§Ï¸«?'Ô¼ƒŸ?°Š¶ï1ã?ïwÁZRÜÇ?°Š¶ï1ã?Øý™N|Ã?·!em|Œ?ã3?XÁž?·!em|Œ?r}GP?e›ýlgàL?ïÛq{dÈ?e›ýlgàLPSR3FGL J1536.6+8331@]z÷@?åğס<À:~†TBwÀ;ýF†Í;¿ì°ç¶Tˆ@ìF±c@ÙH@`˜F¿âD÷\݇¿çð›nª¿æboð9Á¿àâf¾O%AGNbcu@‹¦­À˜$PowerLawNVSS J153556+832614?ïþæã¬ë¹?#™[6¤4?!'Å{d?#™[6¤4?ïڌ-þÉ}?†äñ'Ló?r¹èèýÂ?†äñ'Ló?ï°Àù@.€?}px#Â,?ƒÏÁ°LV?}px#Â,?ïý*ˆÈC¯?(ïÛ®BSä?6«¹ÚxãÑ?(ïÛ®BSä?ïý=Ëgœò?8Ð;Ýk¹?6¢Äì
i?8Ð;Ýk¹?îÿÍS–'8?¯ËÒ%!-¿? *ÂKi‹?¯ËÒ%!-¿?ï0½D¥?"I9¨ïØ?™èWƒ#ÕU?"I9¨ïØ?ï«"ørÝ?ƒô?÷IŸ?…7xþs¬Ù?ƒô?÷IŸAGN3FGL J1537.8-8000@s_<`ŸÀ3}_²?À9CÖNUÎiÀ;~æ"ôï+?Ö!ª°ÔYð@KÚsÿV@}Ç/$Ü¿á¹SK~ó¿ãgâ(Ý"¿àRÁՑ±2¿çœì='AGNbcu@•rdxGPowerLawPMN J1537-7958?ïþôòÛª5?!b¯¦¯? °ÒÈÒ)?!b¯¦¯?ï°>¥ñÛi?']è. P?ƒðV§Î?']è. P?ïÛ¨Ìñ?|#SPcâ?r+ò'*'?|#SPcâ?ïÛ-O*?S\\8?rttàio*?S\\8?ïý/ý¸kÜ?7àþ|h´?6€±çŸm?7àþ|h´?íñGî'ˆ?¶j­0Åݪ?°uÀŒd·A?¶j­0Åݪ?ï¾22W@.?'dqӏY?€ssro"?'dqӏY?îÿ?³Ÿ)Q?…‡à'/±? Å1ƒù?…‡à'/±AGN3FGL J1539.5+2746@Eôv?ø="@Jqÿ΁ÙÀ9O~Rì6À;šÌÜ­?é(·²ù@Ésô–$@©:ÿZh¬¿Ílï)÷}Ù¿à¡_ðÚÕ¿à›Ôÿ˜ž¿æmá|S°AGNfsrq@–Ê{J#:PowerLawMG2 J153938+2744?ïÿx>¼9"?1xƒ¶>"?ø0ÿÄq?1xƒ¶>"?ïáÉ^-\Ú?tV[dÖGŽ?n6¡Ôýˆ?tV[dÖGŽ?ï×Cÿfۊ?sKTt›è9?t^_ ø?sKTt›è9?ïùn©´wt?0Àr(TÐ?JEZ0?0Àr(TÐ?ïÿ=±Ÿ?!ç%¿™ýa?˜XFS#¦?!ç%¿™ýa?ï?™Ûv?¥óæÀ_?˜ÎDœC?¥óæÀ_?ïŸ!Ý»<?‡(‡î×?ˆ7ˆ´B]
?‡(‡î×?ïî¡ëš×?X»|¥e}O?a^voI?X»|¥e}OAGN3FGL J1539.8-1128@v2ï€Uûµ@@çk b
·À9ò¬U^fÀ;s×gZ'¿µc9ìLÿ>@
°R°Ñïv@­Ó %¤Õ¿êȆ)þ¿äj©…䠿ݨ"õèF¿äé£Rˆ–›AGNbcu@§Ö†$Ý/PowerLawPMN J1539-1128?ïÿ6á{ð?' ö—
ó?#Ü"ýå?' ö—
ó?ïÏä%ÑBJ?ƒîê¯7òÕ?x
í!6?ƒîê¯7òÕ?ïÝxÖwè¼?m\Hm¾ˆ?qC"«Éå?m\Hm¾ˆ?ïæ5;ÿ"&?Qe1ÃֈÕ?iÊÄŒaº?Qe1ÃֈÕ?ïý'ؽÏb?7z®¸à«?3i;Êlk?7z®¸à«?îá؛ž<Ó?¡‡G|SS?¡âvI‹ÎÑ?¡‡G|SS?ïŞ…;¾?¬ú±ûÒ×?}0½j_Áp?¬ú±ûÒ×?î§[Cr›~?—ƒk5×H?¥ŠKËiý?—ƒk5×HAGN3FGL J1540.1+8155@]—¿¤Æ@@{¢ò(§À9‹QÿÅHÀ;}êXÎÎ?êú"9!@T6
-?ù¢ºÀèG?ïøœÀ¯K÷?£B†jñC,¿ÛèQHÙ¿°wËNٓAGNbll@¶Y¼j~ùÛPowerLaw1ES 1544+820?ïöN'ï'[?aãã÷¯!2?SbÛÙcjÕ?aãã÷¯!2?ïÓ<&6ç?ƒ"¯ÐŠÂ÷?vaícLZ?ƒ"¯ÐŠÂ÷?ïªèd¿›?ãغï?…EæÓ®õ>?ãغï?ïÃéY»Ä?g
ÛÍ6?~yÓ"Ù?g
ÛÍ6?ïäÑ5^©?jÇ6Žž2?kí.ä¾^â?jÇ6Žž2?îɟLЬð?¯xÄë_'•?£f2J?¯xÄë_'•?îãJê"âÈ?›–kÐ?¡ËQ\õì"?›–kÐ?îõŸV'?–i¶‹&? ¦xö?–i¶‹&AGN3FGL J1540.8+1449@8`Ÿþ7©@Hhâ:¸cÀ:œU5¼À;xÔu§L¿°Çñm<°@DYgzb@ÂgŸÌc›¿áè+ðɬ1¿çPÐò@T¿éØi€¶}¿ª­eÌô¡AGNbll@›c	…ðoiPowerLaw4C +14.60?ïýpÁçŸ?>=ôé9‡m?4yïø°æ?>=ôé9‡m?ïáý¥K˜I?v╋íßl?nZ"ËO†?v╋íßl?ï›êƒZ׬?'™k«¥?‰_0)M?'™k«¥?ïü—¿Ç?0ý•¡Ðê??o‰#ò?0ý•¡Ðê?ïèrhþ?p…'©úà'?gßܙ?p…'©úà'?ï´'ËnJ?¨Ø:\Oê­?œ	o­qn«?¨Ø:\Oê­?î =›¨"Û?¤Ïé'ÏQÂ?­ü&E}ÒX?¤Ïé'ÏQÂ?ﶗ»6ç?{$'b?'Z2ž3?{$'bAGN3FGL J1541.8+1105@3Š"€,á
@Gw±ÿÁìŸÀ9ÊÂñ·üÀ;§À)P[b¿È`®Å›@P‹RY@Þ1àwÏo¿ç>O"ùÝã¿ç
dHI…¿êÛí›=L€¿ïþÉ|w±AGNfsrq@|}£Y5üPowerLawMG1 J154207+1110?ïñâ"ç¼?V hyß?\:×í<X÷?V hyß?ïÏ·"õ%?†Â£LL"?x$nyÑAm?†Â£LL"?ïUâEì°?†º*°C.r?•C·I^Áø?†º*°C.r?ïӜ|DkŒ?`NÖÁÐí?v1Á½}æ?`NÖÁÐí?ïèËè:*b?hâ®jý?g4¨øæ?hâ®jý?î"ôbÄ*?°²*&¦¢?¦°¹Úwrb?°²*&¦¢?ïÐÿ%Z?'Í~Îg,?œeà{TÏ?'Í~Îg,?íp›üþÌ?¨0b %)?·"{!aä?¨0b %)AGN3FGL J1542.9+6129@WØØÀ  @F²`œ˜RÀ7Óû-2h2À:ì³Z§?óòÈê•	½@~b«0E?ýKê"_¿Üؼ'@¿@¿ßû)ñëë¿ßJ:-DÔ¿â½'{Æ}†AGNbll@‰Â>À//˜LogParabolaGB6 J1542+6129?ïÿ	±'ï?C[½÷?ށ Xñ?C[½÷?ïÞQY'?…9	ø+";?pûכ?³‹?…9	ø+";?ï³þc
?"Mbî¡f?ƒyÝôŠÔ?"Mbî¡f?ïó4ŸL•?B{Iò?Y疇­g9?B{Iò?ïþ¿¶cÔ¼?$ú÷,gúJ?$–t‰®?$ú÷,gúJ?ï
¯pùðÐ?²ü	ø½› ?žJۚ|
?²ü	ø½› ?ï¢Ïdù÷?''Ã/Ã|?‡L&ÄñÔG?''Ã/Ã|?ïçê&Ó?`ÿdªq©¡?hÚ©Ú ?`ÿdªq©¡AGN3FGL J1542.9-5141@t~œ…×E@Hm`€žKÀ8Œ7ùk'IÀ:­AÞËÓ?êaV8¾.ò@
h•»=®6@èMß[ð—¿átŠô¿èÝ(œx¾z¿äˆJYj{¿íÒç‹BûPSRPSR@‰×K':)ÇPowerLawPSR J1543-5149?×Q|Zª¬£?ÑM1C?äWAÒª©¯?ÑM1C?å!PW}¸?Èe`•I±X?Õ¼å_Q'?Èe`•I±X?çä|õR?²ë…RBv?ÑÁâ7]?²ë…RBv?æøõÒ}?¤\Õ[Ž2?ÒÙþ[?¤\Õ[Ž2?¼ÞžÜNŸö?ÁÔ¥°ù?ìd,$v,?ÁÔ¥°ù?»4ÐVų?ÁÆá	‰…i?ì™eõ'^ê?ÁÆá	‰…i?ßߖ!®À6?¸·`*TjÐ?à4ï(Ÿå?¸·`*TjÐ?ÄôâN­üÂ?¥ÀMuª?êÂÇlT€Ð?¥ÀMuªMIXED3FGL J1543.5+0451@(|ȵ1¦@E²NŸ CØÀ:,ÅÜÃkÀ; 	Å{Ÿ´¿õºD²6žx@
¸TûÛ?ÿÁàþ¿ëL "ö¿Û±WšŠt'¿âTÃRß̿ĸÞAGNbcu@¨t$xPowerLawCGCG 050-083?ïþ'úO"8?!Ð`'9åú?&àZC
?!Ð`'9åú?ïÂ9VÉ÷l?­>à™u?~ãT­'.?­>à™u?ïÑÏØÙÝ?uEšgß¹?wæõi?uEšgß¹?ïÿꐤtá>ÞÖÛUÀӇ>åoMË>ÞÖÛUÀӇ?ïûþ¯""Ë?@u¼ÝýßÝ?@B‡½i?@u¼ÝýßÝ?ïǪÆ_?¬õGÍ"^?ŸÇ
ª£¹?¬õGÍ"^?ï­mÅïý˜?ƒ¸ I#óð?"¤Žy±Æ?ƒ¸ I#óð?ïþñнG?3låAíM?/@ãTíW»?3låAíMAGN3FGL J1544.0+4938@S̸`.>@IŒÕ£5À:Zäd™ÍÀ<åB¿Ã}}!éµ@'‰¹QÅÅ@j¨_°ٿ׻ϣZ§Z¿àe-Qzy¡¿ëòÀb—`¿Ã‡­,@ŠPSRPSR@qÛô‡ýPowerLawPSR J1544+4937?ïþ»áŽ?%Á@'M?$F%$'o$?%Á@'M?ïî‹è]?làiºÁJû?at+Û?làiºÁJû?ï°×=5Œ÷?yÑTÖüè?ƒÊ0¢v˜Q?yÑTÖüè?ïüÔã‹o?'KY-bu«?;X•"Ï?'KY-bu«?ïüpòí"?:!AܶC?<xg‰Ê¡?:!AܶC?ï­Ë¸®:n?ŽðCc«A?"Ʋô?ŽðCc«A?ïy4 »Y?‹Úªò6²§?Üù"šÚ?‹Úªò6²§?ïܼ[1÷@?jvä'/ùx?q¡Òvғº?jvä'/ùxAGN3FGL J1546.0+0818@0ÄßVø4@FWM@$³>À9°åÜhKCÀ;`üÀ°^Ø?äfIyà[@šÁq¹?û
i€L@ ?ïî
ñº[Ë?çJü©š~Ø¿×XŠå:›¡¿Ö<]ÍÕOAAGNbll@´8JÀƒoPowerLaw1RXS J154604.6+081912?ïý¾ƒw³?/BúsG¤?2æW«?6?/BúsG¤?ïÔ·²‰T¨?ŠA!<΂þ?u¤&º¥À?ŠA!<΂þ?ﱇƒ[X…?ƒ†ÛÉ ?ƒž(!ü¼?ƒ†ÛÉ ?ïËñ˜ç –?d¢å҆»?z3n£	?d¢å҆»?ïûdùn?AãWJ_®?Bo»ºVÙ¦?AãWJ_®?îœ;Øª?¸À¨Àíµ>?¦<Gå	+?¸À¨Àíµ>?ïÛ3ܕ1?Š½Îh7µ?Œ‰3™#Ç?Š½Îh7µ?ï]æ>~?Œ
¶À°…?"C>§Š@?Œ
¶À°…AGN3FGL J1546.6+1812@=í2ÿ0Í'@Hg¥€W©4À:Gç.wâÀ;»Ä4wÖÑ¿Õ¼ùßÄ:@
Yžk˜y@gnåhz¿ãÉÿ&
}¿çf¤¢"È'¿ÐoXÞša¿Þ~K¸˜ÀßAGNbll@™tF§ï²PowerLawMG1 J154628+1817?ïú®ZNˆ­?kP¬»–`Ø?EF—d1²‹?kP¬»–`Ø?ïÐ`¸|ˆ½?•ˆIãò?wÏ£¾L±?•ˆIãò?ïÈ°VcS?yB9ÆÚ¡?{ù§óºÒm?yB9ÆÚ¡?ïû@žçÈb?/Ã$8‹»?Bý…<Åw&?/Ã$8‹»?ïü
¥Â¿?A3¡‰Ê‰<??Oª(–ác?A3¡‰Ê‰<?ï)x›‹‡?¦Ž+è–Jè?šÐì¡f]%?¦Ž+è–Jè?ï@"'(|»?"Å_Í?—훀̯?"Å_Í?ïՂŒül?o¡ßú)8ø?u>¹'yã¸?o¡ßú)8øAGN3FGL J1547.1-2801@u|€àe0@4•2Ÿ|àÀ:MÎ_ªÀ;ƒcÎÜq…?ë'éýÎç@
üF£ÓYY?ûRÄá
x¿ïÍ3Ó¨Dh?ïø5£®h¿á&¸ê¨æû¿ÝG:SZgwAGNbcu@¸?«…¸RPowerLaw1RXS J154711.8-280222?ïí#¸î?iœŒ2ëÊ?bÜäa.ê1?iœŒ2ëÊ?ïu\6óÃ?"-§@àO?'_´¸Œ?"-§@àO?KQÀ›?†Ê4^Yç"?Ž×-.ÿuU?†Ê4^Yç"?îue'?'×>¦ê÷?¨®=ý¿ó?'×>¦ê÷?ïæIxÍyÏ?pæ!ïS^q?i¶‡(çI?pæ!ïS^q?é¨:SZg?ÉDE¨zÖ?É_ã²–b?ÉDE¨zÖ?î«fú9m?{·.ˈ?¥IŸ-È´;?{·.ˈ?ç8ŒÙF?¸»Ïðï°?юæMãsé?¸»Ïðï°AGN3FGL J1548.8-2250@u½¥¶™…@8*% Jù#À9|©žÊ[À;?fg=%û¿Ùà Fåu@'#C¦óÊ@b#¿ø¨ô¿ÙûºÁ1Ž¿äcíÖÝ?¿â¾ŽIj"X¿Õôg25©§AGNbll@ ø¤?åÉPowerLawPMN J1548-2251?ïü¬å£ï?2´`"j_Ø?:Ÿß¼³Y<?2´`"j_Ø?ï˟—?'Ûãb‡Öñ?z0|?°µæ?'Ûãb‡Öñ?ï¹uHÍÄ?Lû$ñ ?¢®ƒlò?Lû$ñ ?ïûq̇=Þ?0ñä'zÄ?B8Îõ\‹Y?0ñä'zÄ?ïøš¼7?MÐFmRÒC?M•{Q2?MÐFmRÒC?ï#pLe«£?¦³A›ô?›'ösJ‹¦?¦³A›ô?ï-'{ú?"û¹µü?š\
ËYU?"û¹µü?ï·äz_ää?w¬‰Ê'_'?'áxÜÜÏ?w¬‰Ê'_'AGN3FGL J1549.0+6309@X9Àgn@EùJ?¿2°À:iêÝYÀ<‹?cÃÀ8‡Q˜y@›@"Yò@Î8£NN¿æ@Ç/ÿÌÿ¿ìpژ½P®¿ÔùT~¡4‡¿èƒdç"AGNbcu@'K՛=ÈPowerLawSDSS J154958.45+631021.2?ïã–U‡×?­hÄsH?liªÐºùT?­hÄsH?ï×u°kÐ?EΌºò?tE'â}$L?EΌºò?ï‹<	N:ÿ?Û+×
?0ýž²ÐP?Û+×
?ïÿñÓ¿I>Ýè-4
4ú>Ýĝƒ€Š>Ýè-4
4ú?ïþ£—|çe?'8¾è±U:?%ƇSoÀ>?'8¾è±U:?ïUžÞZœa?£¥m­'+?•L$=CyÊ?£¥m­'+?ï;‰«ºÙZ?•BÌ¿r‹?˜ŽÊÌ>¯?•BÌ¿r‹?ïþ	Ïâ?4ÁÕGã/«?/¿eQa{?4ÁÕGã/«AGN3FGL J1549.1-5347c@tuè_ÐJ0?Û¨h r2ÅÀ7p@Õ³%\À9ý"'¤?ò1˜Ä1²@ŽG…z©@xǟfb5¿ä̬¶¬Ï׿èD®?îØe¿æïçCp˜¿ïïå|OTHERspp@ßêüÎXPowerLawa?/S+€tJ?°ÝáÛ?ï…fmž?°ÝáÛ?̏cÜY˜ß?ǒꦰ)?èÜ'é™È?ǒꦰ)?Ó¸)wGµ ?´õ婸V»?æ#ëD\%p?´õ婸V»?݁·[g?¯5‡$´ü?á?$?qÒM?¯5‡$´ü?'çï¸:?ŸÃßÙå?ïpǘ°eŽ?ŸÃßÙå?¡®î(*«?²Lzøô¼ä?îå?¾å?²Lzøô¼ä?Ç
ÙOš¥'?ºB–†m?ê<‰¬Vœ?ºB–†m?²òʬCçÍ?š|ã!ð7-?í¡¦ª'ÿæ?š|ã!ð7-PSR3FGL J1549.4+0237@%¸çÖyõ@DtÈßØBLÀ8j™ç2«À;UýgŸKŠ?ÛÑ^$@ÑIOL@´é •vÊ¿å;ßÊÞ鎿æGkX,€«¿åÉ_›'8:¿ë:ui0AGNfsrq@êаò{³PowerLawPKS 1546+027?ïüãZ—ë?6¶®äj´e?8äî÷4Ø?6¶®äj´e?ïÓ§œä?ˆxŸ«Ç
?v,uKªý?ˆxŸ«Ç
?ïRK"ìA?ˆ,:©(–?¶ˆƒ?è?ˆ,:©(–?ïø­õ,x•?3º¬Q`÷³?MH+xrtÒ?3º¬Q`÷³?ïûIZù"?CËh!")é?Bڔ†ŽŠú?CËh!")é?îÑû¥ÕP?²¿Páýˆ?¢àE®î'?²¿Páýˆ?ï5_iG?"MJ[Ìb?™^4¶U)?"MJ[Ìb?ïÜñ½>†Æ?hÌZgP?q‡!hû­
?hÌZgPAGN3FGL J1549.5+1709@<ҏÃæ@Gç
€CRÀ:–ŠQýù–À;ג'µP¯¿âjڋə´@f÷ºâ±?þ¨›ÿÊ{¿ë;iå™CÖ¿ÙS'Bï$!¿àü¦Mÿ^½¿È´q'¥šÀAGNbcu@²EîBZîcPowerLawMG1 J154930+1708?ïÿ<€äÁá?–aã§G?oá÷¦?–aã§G?ïà3ÿ¶Ùñ?{'JÀK?oÌRÄö¥?{'JÀK?ïÖLYc¸P?{(²;%ç?tÙÓcqká?{(²;%ç?ïÿ¸<G>ó˜÷\.3ï?ððläjÙ>ó˜÷\.3ï?ïÿ÷з?¾F.šYÅ?!.ñXã?¾F.šYÅ?ï1,ꈎH?®Wgiƒ?™Úb·…<ë?®Wgiƒ?ïÆçÑ=¨`?~d{Ï·?|ŒLŽ(@?~d{Ï·?ïü¹ÃŸkZ?9l›-#¼?:1äÃ
?9l›-#¼AGN3FGL J1549.7-0658?ó˜OÌû@A¾ß¤?æÀ9;´L£FÂÀ;DD<oò׿î求÷õ"@ëUN.?þÇÑ`w‰¿ËðzÑØO¿àkI]ǟ¿â¨ëy5K¿ÌØ¢cÒ§AGNbcu@§‡g¯·éPowerLawNVSS J154952-065907?ï@ü¹=?ŵ°DUð?ŸüÞ±
U?ŵ°DUð?GëÛ?¯(«¹6?‡œ>ê•mb?¯(«¹6?îöͺ£7?ž"Ù>´Át? "$a=š†?ž"Ù>´Át?ïÿ—í>~¸?FLWw#†?
­ç[‡?FLWw#†?ïö엲'Ÿ?T`Ùak6þ?R&Ðþ¥î?T`Ùak6þ?î='•?À²E¹{?¬&æ³M«Í?À²E¹{?ï5jVFD?—HëH'Rô?ŸYR¼oy?—HëH'Rô?ïù3vé°!?KxÑGÖ%Ó?K2#1¥ô?KxÑGÖ%ÓAGN3FGL J1550.3+7409@[8_á'p@B×@&`½À:oË
Tí˜À<¶ŸcÝö?á‹b¡àºë@¬P¥^ô­@›@bƟ¿æz\q½T¿î1=#:Üd?·ß¿¥"F¿ãìüÝAGNbcu@€ëæÞüz:PowerLaw87GB 155014.9+741816?ïÿ­XN†Ý?@÷ø>Ó¸?©ëÈÀ.
?@÷ø>Ó¸?ïÛ¨cУ¶?}üï‡ >?r+Î%l•?}üï‡ >?ïäÝj²Y?p
Óã?k"•,ª´p?p
Óã?ïçÄ>«-ã?S@—¾XÛÛ?h;Á/¶U*?S@—¾XÛÛ?ïÿ‹ÈÂôS?vµåÇXU?

ۼDZ­?vµåÇXU?î֍v(Xí?±OíHÛJ›?¢—(žVX,?±OíHÛJ›?ï¤z¼<dh?‡"p´ëQ?†áPû5¹ø?‡"p´ëQ?ﺌ=è?|Šøýq²?\ðÀú¶?|Šøýq²AGN3FGL J1550.5+0526@,gÀ_A@EÜà@GÀ8à€If{_À;n"aKts?ílÂ|*¸@&wºL@¯ñ⢿Õ.J ã¿æáNö‡¿â$à"¿ïþÄö¶ørAGNfsrq@ŠeÉäPowerLaw4C +05.64?ëÔ5¿T",?¾]˜!ˆ¬?À¯)­¯P?¾]˜!ˆ¬?éWSÒÂó?ËG…8O€?Ê¢°· ô4?ËG…8O€?éÁŠ÷Üú?®¼q«-?ÈùÔ#Ќ?®¼q«-?çf$Fl‡?©mk~®OÂ?Ñ3á·s&ò?©mk~®OÂ?áQBÇó®?ÏôéÈjâ?Ý]zpÔ¤?ÏôéÈjâ?߄–?ÔÆ4Š˜?à=´üÿøý?ÔÆ4Š˜?àß~ÀÛË?À|Aw¢+—?ÞAÈHj?À|Aw¢+—?ΔÈ,1¿É?²¸ÊÝ‹?èZÍôó?²¸ÊÝ‹MIXED3FGL J1551.1-5610@tae¿­)™¿ù­1@ê«ÛÀ9²`9ü{À:" z^jï?í·ºbM8S@Ë îؐ?ü ¢qON?ïwÌT×È©¿X3¬Äˆtr?‰7º£ÌŸ¿Öþ«OTHERspp@ÆdBñ©ûçPowerLaw?ì§àþZ{?»Tϐ Ÿ?ºÀø=,(?»Tϐ Ÿ?î6.€?º)È÷ç=ø?¬ŸÍk"î?º)È÷ç=ø?í–¾¡?§¤Q_llÓ?·óJÊø?§¤Q_llÓ?îï
}RLd?…™9ò·?¡(*Û9¼?…™9ò·?éYGñ
ý?ÂZ{Ý­+?ʛêà;È?ÂZ{Ý­+?æ@¸ÊêÒû?ϕ§Jöã?Ó~Žj*Z
?ϕ§Jöã?ì©ÓÑ"òÉ?©PGlÛ]z?º±avèi¶?©PGlÛ]z?íӓ5&}m?ž
Õ­,Y¶?±cfUF˜?ž
Õ­,Y¶AGN3FGL J1552.1+0852@2q_¾¬y@EÓ7GMœÀ9õäžz©êÀ;¯%v²?¦šXmjÁ´@ÿ-ªˆ)Z@®{`sˆ8?'`ÏÅòàT¿ßŠµâ5ÐÙ¿éñ¡À¯ˆ¿àé¡r¹–AGNbll@–ž"©*0UPowerLawTXS 1549+089?ïõ·I­Èü?bãwH2â?T'l€²$?bãwH2â?ïØ(â­°?ƒR;Š½W=?s돆€?ƒR;Š½W=?ï)ø	o"?'^Ì×1#?šÀþÌôñÌ?'^Ì×1#?ïÞÔ¿4ˆÉ?[%;€	&Ò?p• }È߁?[%;€	&Ò?ïªjÉfT¸?Ë·Š+£®?…eM°¹¦?Ë·Š+£®?î{ñŸâUm?¸Gý5C…p?¨@涐6?¸Gý5C…p?íJÁVðÓ?«Jàß4u¬?µ©õO€yk?«Jàß4u¬?íûÂQ¯Ü7?¤o`Æ)Ø?°!ís]D?¤o`Æ)ØAGN3FGL J1552.9-5610@td•`"¥¿ü#pÀ\|À7'¨|‹kÙÀ:LÔ¯]Ÿ?Ö.]pžx§@}Ñ2¸$@@YŠ¿Ýw¨Ãƒ"	¿ãÎ6YXa¿âo¥ßøù|¿àŠÝâɹOTHERspp@£.¬1PowerLaw@?ç50ÆÇO4?Ò×O÷Üg?ѕžrqa—?Ò×O÷Üg?îRV'ˆ?¸|3j™.˜?®ZÚ£òZr?¸|3j™.˜?æ¸Õn±äi?¶&~½Co?ҎU"œ7.?¶&~½Co?퍔&#fs?×/Äl?¿?³"^Ð.¦è?×/Äl?¿?â…y«VtE?ÑÊoK"¤V?Úõ©Sw?ÑÊoK"¤V?Û¹ÿç< Ö?ÐÖû
k½,?â#a¯•?ÐÖû
k½,?é@BƒïI‹?³gÚ´àՕ?ÊþõðBÙÖ?³gÚ´àՕ?Ü:Pò‹×?¾ó|'Að?áâ׆ö:?¾ó|'AðMIXED3FGL J1553.3-2421@u¸ÚŸ¾vÉ@6Z(Àª'À9YêPkR^À;WªÒ§a?éwØ?á[>@½¸Ûÿ@<_":4¿Ì[>¿çÓSà¸ù¿ào ½Ëä+¿î,º~t,ÖAGNfsrq@'}¬¥zxlPowerLawPKS 1550-242?ï…ÀògÖ?Œå¦º^s?Ž¼ÏԔx?Œå¦º^s?ïWT]­ã±?¡*EG²i?•tCdQæ?¡*EG²i?ìSiðšÃ?¨Æ'=]BK?¿Ed°{)ä?¨Æ'=]BK?í÷Ñ?Î!6?‹(^<"$€?°AvüéÒ?‹(^<"$€?ïgÿôþ€_?"õ¿>¬©?"açÂ?"õ¿>¬©?é")£'z?ÈcH*Ljù?ɳYs¹¶?ÈcH*Ljù?êúK¨n?±†9Ö?ÇüÓù^H?±†9Ö?åCdÆ«©?´ò'ÈÞÅ?Õy7îr¨®?´ò'ÈÞÅAGN3FGL J1553.5-3118@uieà.©a@15·?œÎÀ9…àãÛKÀ;Oûx±Â…?ø(0…ÙÉ5@>4r"‡>?"3/ë¹Á?éÇW±(Ó?ïû¡ék¶T¿ÓSM©oê8¿×æõU_¶}AGNbll@²ìÈr° ÅLogParabola1RXS J155333.4-311841?â1±šä"·?Ô<ŒMUÉ5?ۜœÊ6֒?Ô<ŒMUÉ5?çh£AýÀ?ϙg¿ÌN?Ñ.z¹|€?ϙg¿ÌN?å5ï™3ñ?µô_'z:?Ք ͙À?µô_'z:?檈K,h?·™â_s=?Òªïi§/ý?·™â_s=?éf3[¶!?ÇÉáS?i?Êg2''{?ÇÉáS?i?Û¼»7#,Ö?ÓyúE3™h?â!¢dni•?ÓyúE3™h?é¹Ø(u•?µ!5ñÖ?ËÝŸ^)¬?µ!5ñÖ?Øè® øï§?ÀÇ+ËéU¢?㋨¯ƒˆ-?ÀÇ+ËéU¢MIXED3FGL J1553.5+1256@7ɁOP @Fœ  0÷ðÀ8;‰‹.œËÀ;8±0?õÄ>£©½Ô@÷A\k»»@ÅÂnoI¿â]ÜT)¿ä")y1U¿ç+µª¾§h¿éÿì²£ßKAGNfsrq@€ëíúCþLogParabolaPKS 1551+130?ïîÆg_$?^ô[paçz?a9êiæ,«?^ô[paçz?ï×Y_0«Þ?ŽÊ"J?tSP^(ö?ŽÊ"J?ïHñq­þ?"Æ\"ô)f?öáÕ9Ü.?"Æ\"ô)f?ïïó[½ý?FÈÁ!íD?`¤‰Óè?FÈÁ!íD?ïÙ§"*°?pó[ü-ú?s,nÜÎ?ó?pó[ü-ú?ïÕÆø?«ŸÜzÊ	?œeG=½a?«ŸÜzÊ	?í›gá þ?¦9…QÂl?·$À?¦9…QÂl?ïÞ2
Kö?g§Mþº×i?pæùn¢gL?g§Mþº×iAGN3FGL J1554.4+2010@@ÐÖ 2¥o@Gß<ã.À:E‰bÙÀ;Êô¯iåw¿ñSÀßIý@–Ehƒ@¢à?Ee¿æa‰iÃ	¢¿âԗ.Z[k¿×&;ìϿ簛µ
ú{AGNbll@š»6z—PowerLaw1ES 1552+203?ïûßR%Õ?Ayvþû–?@'¶ýýL??Ayvþû–?ïÙR'%
?ƒ"(ÿC;?sw֙0ëi?ƒ"(ÿC;?ï¢5ظ,?"¢ÓxÙ?‡r¹<…?"¢ÓxÙ?ïý»?&ÍO@­Ò?3‡ðŸâ7Î?&ÍO@­Ò?ïëL~¯Í?fõbDjá?d³âtñšë?fõbDjá?ïFz·]?¡&æ$µã?—-ð¢@¼q?¡&æ$µã?î'ýãgT?¢Ñ4µ6?¦Ð!Ɇú¹?¢Ñ4µ6?ïÎ$íŽýù?z*'IA$?xí‰#3oœ?z*'IA$AGN3FGL J1555.7+1111@5ë€uf@EúÕߛªÀ6‡ÜŽá¯³À9Øoàb«Ç?ëXlQ?–@DGw7ïÛ?øO÷øµ¿Ñ$¹»Öô¿ÚbR'¿Ñ§—U"þ¿ÑAЉ3´§AGNBLL@—M…¡ÊÀƒLogParabolaPG 1553+113?í°sOÙ?Ä_G+À^?·÷Ê{÷º?Ä_G+À^?ïß¼ð£Û?xñil'?p!ü~*b?xñil'?é[:/'?³Òp!Ôz¼?ʓÏCc?³Òp!Ôz¼?ïá/£º7?_!â:–?nàÐ̨×?_!â:–?ï2øp)¥?¢Ž—Dý?™ ññ'5e?¢Ž—Dý?ï?ãDÞV?«¦GzX"Ó?Ÿ˜•¬g6?«¦GzX"Ó?î€E,&q?¤ÜÚ1
?®÷û©Íüõ?¤ÜÚ1
?惘¥Ù!?¦63»gÎ?…^}$H'Å?¦63»gÎAGN3FGL J1557.4-7040@sÓIàâiÀ*QGàiaÃÀ9²ªÿ«1À;¦™_·öÀ	)^€"ä#@çÊ´èª@h(ÿӊV¿åx­Áä}¿â¿"nÑ3¿âÐ*æô¿æg¨MðŒAGNbcu@'˜ø -àPowerLawPKS 1552-705?ïú: ÀÈ?J*Žƒ¤€?G"?
3Ä?J*Žƒ¤€?ïÊ/M—ÚÊ?‡*]‰Ž'¼?zèY)ÃÇ
?‡*]‰Ž'¼?ïÈsvÅ.H?{kŸúöo¢?{ÆDŠÚø&?{kŸúöo¢?ïÿÿq1=>›Øù¢°$>'ܾ±)é>›Øù¢°$?ﶮO´S?ƒTü'$?'Tl??ƒTü'$?î˜\]#¹?´`'€µ?¦z:0aùn?´`'€µ?îíÃn÷{ï?˜F¦*í+¡?¡#Éd(	?˜F¦*í+¡?ïÿàrÆñì>÷1Œ5
›>ïp©¬eŽ>÷1Œ5
›AGN3FGL J1558.9-6432@tøŸƒ¾fÀ!GŸÕó½À8ÉÄ<ÛR¢À;@cÞÌ©'À¿^\¶@fƒÂ—¿¥@0K`{•Î¿æ륙=dv¿Ö†§qüû¿á}PPB¿ÕÚiýc‡SAGNbll@ ìºŸ¾vÉPowerLawPMN J1558-6432?ïõþOYb%?Jd¬ÐÔZ?Ta]¹Ö½?Jd¬ÐÔZ?ï¸FÏ-‹e?Qւ[}?îL(–"ä?Qւ[}?ï»)®œ'z?€kEÙ¶
?5"Kxç¯?€kEÙ¶
?ïÿþD‹l¨>«ëþ*C>«ºͤœ>«ëþ*C?ïæÞ<Є¬?aß÷Ï=k?i!Âì"üM?aß÷Ï=k?íJæŽûí?Á6YK~a8?µ¨Ë‰jrF?Á6YK~a8?ï6i'"^5?"Í]ƒxKê?™2ϲ›£S?"Í]ƒxKê?ïÿÆÛWeS?RŽ³ówz>ü'Xg—}1?RŽ³ówzAGN3FGL J1558.9+5625@UäÉ$.@FàxÀ>-À9DËüÃ4žÀ;´Sø¥˜«¿ñmš}[F@éÊ@®êÖù¿çè(Z½ë¿Þ–÷Üá¿á·_öW,¿æŠt¼P¹èAGNbll@–Q$Ý/PowerLawTXS 1557+565?ïÿ¿¢å9>õÀ>Á€û¿?>u¹™J>õÀ>Á€û¿?ï׈TÍ·®?‰F)CÁ?t;Ճ&¨ó?‰F)CÁ?ïëðÈßØ?eO_•?d7ЃÀ?eO_•?ïÿ¢Ôù
•>üãa*X™ã?J´žAœª>üãa*X™ã?ïÿ€},ÀA?-¥­Ä³^?à¹ZÇ 6?-¥­Ä³^?ï^ÞãƒP5?œfxøÞ ?"$#ˆ¶Át?œfxøÞ ?ïݱUÅPÏ?yI1¸6û-?q'U·p…?yI1¸6û-?ïúô\ç??D`y;3¦?EÀ.:y !?D`y;3¦AGN3FGL J1559.7+8512@]·Êÿm3	@>TDŸlArÀ9ŒO"}ŠÀ;䰔‡áá¿ða5Tu£@{=gµj@ϊ¿Œƒ¿æØß/®vÿ¿åõ³ö3šÚ¿ß´2¿o¶¿é~ªùF&AGNbcu@‹•1ŸŒ¨PowerLawWN B1609.6+8517?ïûÊíy–?@Yv~Õ?C¨ÓÛ° ?@Yv~Õ?ïڜYΎª?ƒéÏÃsq
?r±Ó;ÂÊ?ƒéÏÃsq
?ïÞA2zQ?qdÍ)Œ›?pý_EƗÙ?qdÍ)Œ›?ïþ¡|H?
R@ÎàÙ?%ï
jõÐa?
R@ÎàÙ?ïôd|	‹?_˛ޑ?W7fÁ)$?_˛ޑ?ï%25ÿŽ?¬i=k§`/?œûYµÐrN?¬i=k§`/?ï^RÀ¹|?'ԏ;ù¦?"5§íõZm?'ԏ;ù¦?ïæ–NÃT?e'Œ©?iiéõôÛ¬?e'Œ©AGN3FGL J1559.8-2525@u¾q'l@4'	€²BÀ:lÚÌiÐ~À;ž
ø†¿ã
U€1‹
@€wö[¼i?ÿ-€kË*¿éäåŸxù¿å^â8³•¿ãK±së?­-ZoüÖïAGNbcu@µ ³3333PowerLawNVSS J160005-252439?ïþ§µ]'Î?2àÓnç‰?%"«Æ€«á?2àÓnç‰?ïÊ®ëC
$?ÊÑ}"3?z¨ŠG]?ÊÑ}"3?ï֒ýYmÁ?oöº]f¾ø?t¶Liç°?oöº]f¾ø?ïÿ)¢ª~2?ÐQá}?˨ÞW¦?ÐQá}?ïý2,îÔ?=3HKP]?6nÈm±È?=3HKP]?ïø
é™?°ýjw¸¶?@þÀhÞ?°ýjw¸¶?ï¹ótèp}?µÔÖæ?ƒ"ŋê¡?µÔÖæ?ï눏}?dâžàžBx?dwî[åDm?dâžàžBxAGN3FGL J1559.9+2319@CTÇÀ'á@G¸b`GhtÀ9玦 ™À;›Î­wœð¿â"'p³v@µ
eÄ*@ÍÏڀÀ?íÂÀÜÿtë¿á-v"q¿äPcxSŒ¿Õðï
(;ÍAGNbll@¡-\ú¬ÚPowerLaw87GB 155744.0+232525?ïýýÀÏWZ?3¯6¢Ü¦€?0ú¾¡Š°?3¯6¢Ü¦€?ïÜÕřÓ?ƒ$µäJdJ?qö•3®?ƒ$µäJdJ?ï¦!d©¢Ñ?"~ÿ®Y@Ï?†w¦ãU»£?"~ÿ®Y@Ï?ïþŠ«Pa~?èù'Ü÷A?'UIkâ6«?èù'Ü÷A?ïüÃڂ9x?<š«‰XP"?9á*[¦?<š«‰XP"?ï~"HT?±<~•ƒÌ?œ°/}ß
s?±<~•ƒÌ?ï\CÎ>šx?'uߧ±9'?"w†4½?'uߧ±9'?ïîKZS?^Ù|ޅ?aÿ´e(Ìó?^Ù|ޅAGN3FGL J1600.3-5810@t\3¿µÀu'1>À9ìæ˜Oí~À;KRü&V¬?áE'ÏiÕ@	d^¤P,@Ô?\â.¿âÌ Ë¸¶Ñ¿"îj+lë;¿æ}†Ev¿àpLžÀ—AGNbcu@±8C@N¤©PowerLawMRC 1556-580?ïâÕ¾ŸÎ?€ñô݋®™?m*A?åò?€ñô݋®™?ìÙb~Ç©?Ã[HþÃ?¿É4ì	»?Ã[HþÃ?ï3ˆ"¸$ä?'µâCHs?™Žïoڛ|?'µâCHs?ìAሊlo?ž'ƱÍ?½ð󻬜‰?ž'ƱÍ?îÚÇ
ãUG?¦ íTd'Í?¢SU:GŽ?¦ íTd'Í?˹ÖÊkbh?ÊÉ:
Ρ?éŠMe'f?ÊÉ:
Ρ?íäÿ~Ø?¨xl-µ?·Øä;A?¨xl-µ?Òä+æ/@Ø?»É_Íù{4?æêè_"?»É_Íù{4MIXED3FGL J1600.8-3053@uzÿ°Nè@0uS€°"ˆÀ9Цã.8À;É,.\4?÷>¸ŸÄ+@PRþª•?òšª8"[J?ïþ+«™:=¿Î²¢¹ÑB¿ÞTn#°¿ìbÇÒßWáPSRPSR@¤ݗö+PLExpCutoffPSR J1600-3053?ÆQšk?'ç?Æ,O£E-Ë?êk™e0F?Æ,O£E-Ë?ѐvbæ\É?Ë&._[Q­?ç7ÄΌћ?Ë&._[Q­?Ûv¿lën?·'Cé2´?âD 1IŠI?·'Cé2´?ÛáN}Ö3?±šJ
é|¬?âzXÁæ?±šJ
é|¬?¤öíýÅ?®"‡w)Ãx?î¶ Ÿã?®"‡w)Ãx?»úÁ:J ?Â$"Cz?쀧Ü8¶¼?Â$"Cz?Ĉ0?²‹®èhè)?ë\º:ÎÝô?²‹®èhè)?¹J@õKm¨?¢øï"Í?ìÖ·ár+?¢øï"ÍPSR3FGL J1603.7+1106@7ôàM/@EfÀ(yœÀ9ÑøQÆÀ;{Þ-G`è¿©­‰ô1«ú@,f…›
@˜¿aÕ2¿Ïû/i¿æÊ-ªL0¿ãÕÙE"–O¿âïHïíAGNbll@–Æs3333PowerLawMG1 J160340+1106?ïþñÂÐt¢?2ùéÁGY? ãÔÊçB©?2ùéÁGY?ïӎ~Í)X?†æ@öìæ?v8Àž:È?†æ@öìæ?ïÅÚ"¨ê?~v9«dù?}ÿ#J?~v9«dù?ïú¦Ël‹«?-€¯ø?EdÒ*eŠ?-€¯ø?ïþË<~á\?&ø<(?#L7…-l9?&ø<(?ïAóy?«¥ÿ]·£í?Ÿ÷݉Âé?«¥ÿ]·£í?ïma–·«Â?ãÒ3$UÜ?'SÍ sÇ?ãÒ3$UÜ?ïÔaË:ë'?lEeP˜õ?uÏSl$s?lEeP˜õAGN3FGL J1603.9-4903@t™€o&)@Œn¿{UŒÀ6üUFƒrÀ:Vól|*?ÖØÛ~@w¿@ˆY«B@«ÿøž7¿ã\̀—¿ä©a÷}
Ô¿àš¹yÞ¾<¿Û+I¡AGNbll@™ÎË]ÌcñPowerLawPMN J1603-4904?ïLªÌƒ ?¯ë1ÅRŸ?–j¦l.à?¯ë1ÅRŸ?ïeg|ªº?®nì}pT?SÚD³?®nì}pT?í–Õr]@?¨ €ú¢"5?³IWMHý?¨ €ú¢"5?ïüŠ>ª,0?)B©}{—?;®1¥®b?)B©}{—?(ߍØ?ŠºëÑ¿S?€ÝÈÒ°?ŠºëÑ¿S?ìý¤¥³¥¬?Ψ­f]¶?¸ÚÑø$?Ψ­f]¶?íïÜÉfˆB?¨º¬ª;ª?°³ïÖô?¨º¬ª;ª?ïñºÁÌ,ƒ?R÷i`"f?\Š|Ýىÿ?R÷i`"fAGN3FGL J1604.4-4442@tòߋr@|€.8£À7µ"k4+À:ÃÝo²?ƒ?çðû"'\@7£9€A@Ÿ­@j~N¿ãª]ÒÝÍ¿çå)MèQt¿ã–È6¿êÔí¢QÆiAGNbcu@†§ï²-PowerLawPMN J1604-4441?ïú0wŽyL?TŽ¶–|g?G>"ˆ·à?TŽ¶–|g?/
º?™ªci§{"?‰ôK=p?™ªci§{"?í¢;%"­?¦ªHð2"T?²ï¦(Ž¸—?¦ªHð2"T?ïîeo+Ã?Gg䮐V?aš'w ?Gg䮐V?ïõ2'W
¶?\Rg2"Ô?UšÛ(©C:?\Rg2"Ô?íû\€:î?¹'ZE*]u?°%ý¾Z?¹'ZE*]u?íɎ(ø?¦ÕW¬÷?·á²²Ñ@?¦ÕW¬÷?ïÀš;¢dç?qçPÜé[î?²â!¿¼?qçPÜé[îAGN3FGL J1604.6+5714@V(Àª'@F]K 'ßÀ8¦'w"ŒÀ;'ìÝ
?õ"AöðaÒ@•‡û6——@žð86Ó&¿ßŽ8	¿ç?Î)̵®¿åò.XŸ¡¿ë{ùJ¯&AGNfsrq@€m=…œLogParabolaGB6 J1604+5714?ïõÎËwº?Pçígœ¡?Tbh¬D·?Pçígœ¡?ïÏÝU}'?'†
VúI?xy']€NÈ?'†
VúI?ï	ü™ªFÌ?'n+ÿ"º‰?žÀlÎ&Âv?'n+ÿ"º‰?ïV¸€åm®?s¬1´?•(ïãRJP?s¬1´?ïðµ‡_£?b¥á®æ?^"ñí'IÓ?b¥á®æ?î· ¬C¦"?­Ì6‡£
?¤…õ:
ÉÀ?­Ì6‡£
?î
;éÔß?¡E´#h?¯^,>Îý?¡E´#h?íž1W? å'(î'?³"šË? å'(î'AGN3FGL J1606.1+5630@U̚ÑVŸ@Fdä`gHäÀ:~À?öÀ;ë¼Õ±À $rÑç@Þè<k?ÿ'N^²½Ø¿ã«;þ'sŽ¿èbÅ'øþ•¿ÜÄò]€
׿ǯLý£sAGNbll@°¥E\)PowerLawRBS 1558?ïÿ‹˜úã6?-?
¹ûÉÏ?-?ïåÄgE?r'<…jV?j;˜±a`?r'<…jV?ïݐ@?yÜÛvªt'?q~·Ä¾'£?yÜÛvªt'?ïÿþÁBû>£ÂãDmMÅ>£ðF=h1Ó>£ÂãDmMÅ?ïÿAS²Y¯?Ê	x›">?ՁLJê?Ê	x›">?ï<qfäTm?©–æä_—i?˜qÓNq?©–æä_—i?ïÙ2öVÔ?z
¥'pÍ?sf"ìÕÖ?z
¥'pÍ?ïÿÏ?æl?ðÈDÇ'>ø`(+KN—?ðÈDÇ'AGN3FGL J1607.0+1551@=`A€ÓÏö@Eµëž*ùÀ8kğס<À;]_Âví?꘴îDýÇ@çL‡`\@F¤‹¿á—:2›¿äE0X.ã¿äñšÃ‡¡¿æB7Š°ÈŠAGNfsrq@‰.]á\§PowerLaw4C +15.54?ïåºJê	?}ñ
ÕÊ?jãEۑ–­?}ñ
ÕÊ?ï=ÊÏ­¸ò?¢ÂX>%€?˜F¦ßçÃ?¢ÂX>%€?ïžüÚSœ?ˆfA?ŸÙù?ˆ@É|häÎ?ˆfA?ŸÙù?íMà-Û8(?–«|`œÐ?µþnpÂ?–«|`œÐ?ïsÙI:&?—W¬í¼å?'"ÖÜ·F?—W¬í¼å?ê¬Ó§Ô½)?ÅAááE?ÅL±`­^?ÅAááE?íÜΠj ä?¤ÛìVS??±Šýìb?¤ÛìVS??àôH1YX?½Ä{Á'¹>?Þo՝MP?½Ä{Á'¹>AGN3FGL J1607.9-2040@v, <K
@6""?À9½¼{À;bYG™ò…¿'0ÖÔcø)@
c-ÜÝ<@?©c;¿Í2=¨4ō¿àæNè订¿ØØ©òçz¿ã²öЉùFAGNbcu@¨"Aaä÷fPowerLawNVSS J160756-203942?ïýïëœ?1¾šüYžJ?0€¢¨ÈÏ?1¾šüYžJ?ïɊôòî?Š´:+­Q?{:…üE˜¶?Š´:+­Q?ï¼zZAȀ?|HŽUÂûû?€ái^·Ê?|HŽUÂûû?ïÛu)!âS?U²›QŒ[	?rEk'L¦m?U²›QŒ[	?ïñr•ìr?_]¹¥òÓ%?]Ô©"k??_]¹¥òÓ%?îh"Öû¾—?ºÕÛîlž~?©v°aš?ºÕÛîlž~?ïŠGgÙ¿5?‰$C"öù?n&ßÀ?‰$C"öù?î˜t°Ö÷ô?"8^$ÕJÀ?¦x´ñ´™Â?"8^$ÕJÀAGN3FGL J1608.6+1029@7ÿ·ä@Dh _ñØÀ8‡ôafLeÀ;\¤£¸×M?ôXO´HG@_óWûêr@óÑ@yí­¿æˆ{QZÁ¿æû…å\»˜¿ë	Jƒu¿í¯|¯AGNfsrq@~¯£¢œwšPowerLaw4C +10.45?ïá8Y°~?kS:fD?nÇãŠÒ¢?kS:fD?ï¦tÛ
5?––u\T?†bÉ.ú¾?––u\T?î–YJk€y?–jÕ@K»?¦škZ#ßo?–jÕ@K»?ïShCš?°•‰<Ì?ŸÕ'û(Â?°•‰<Ì?ïæÌ*™b?g
W<"ë;?i3Õ$ùe?g
W<"ë;?î"V}Kk?µÒ?ÀnÌ?®MڙãF?µÒ?ÀnÌ?î™YWV m?Ú¬<0Ý?¦jjˆÞ+1?Ú¬<0Ý?떿£sž?¬©4*ú¶‡?Á¥ár1‡?¬©4*ú¶‡AGN3FGL J1610.6-3956@u3¸Ÿƒ¾f@ þ{ßõH—À9ä@†ØÍÀ;
þ®Ç(?Û>ëÙÛ@(¬~¨@áé€aº/¿çþöjªï¿ét¢ #¿æZ||¨¿ë§"÷ 2zAGNfsrq@€Î4mÅÖ9PowerLawPMN J1610-3958?ïA
$UË?œ(GJV
Z?—ÞžXª®?œ(GJV
Z?ï%ÝæC²?¥
:_©1?›DGŒïWµ?¥
:_©1?ìÿòIðI?¥Qƒ/"Ï'?¸m±Èà:?¥Qƒ/"Ï'?î 1Hwh?"ÈÉ·^q?¥üëuõɝ?"ÈÉ·^q?ëà"CeŸ0?¾ŽæÌà?Àvòiƒ@?¾ŽæÌà?æ
«øº?Î,ˆÌ9Ks?Óä©ÒƋ?Î,ˆÌ9Ks?èy>a?¶ÉÎ^«¹?Ïç®ÿ}?¶ÉÎ^«¹?ãÊ'¸D™Q?²ÝE;A¡??Øk°vÍ^?²ÝE;A¡?AGN3FGL J1610.8-6649@t™÷LÀ&J§€âéoÀ8[#'Õ€À:ìHŒ`Ì?êm¹'~[6@¤­ùwû?ü^¶­yö¿ÜxŸ
Î2¿ÔwFÀP4¿Ú»¼œpR¿Ñ3þÜáº<AGNbll@ª9?|í'PowerLawPMN J1610-6649?ïæ&wZvæ?i'cãÔÏ?iوʤáo?i'cãÔÏ?ïf¹Þf/è?¢m¼q
d?"(Ä,ZÊþ?¢m¼q
d?ï®°(ôS?"±\ðü.?"Sõ·-ÿo?"±\ðü.?ï'=Uÿo?kç¥ÿx-?‹¸ðª€$[?kç¥ÿx-?ï±<õd?†‹¦Û¯:?ƒ°Â¿P	?†‹¦Û¯:?ê'zy¡_>?ÅGqªM'%?źzƒ?ÅGqªM'%?ïG¿"¬?—AðOӌ?·æ '?—AðOӌ?í°Ø&¿~Ó?š¬:"Ì;ˆ?²y>ÈL;k?š¬:"Ì;ˆAGN3FGL J1612.4-3100@u¥ 8L@-JÄ!, rÀ9ÌÎFImÀ;—A¥Ãt?öCÞâ# A@"1jÜí?èÆ£É&Ð?ïýϘÑj
¿·l'ðû!Á¿ãÊ"Cñò¿åàÜ+íøAGNbcu@¢ôü¹#£LogParabolaNVSS J161219-305937?íÞöÑ5Ž?À¸·
•6?±Ix	 ?À¸·
•6?ë¹Çö|?Å+-#`û?Áã¼'Ž?Å+-#`û?çLš
Ev?µïã« '?ÑfË×ëu?µïã« '?éôºÀÁâÊ?«CM¨AŒ™?È-üøt×?«CM¨AŒ™?éÊT9¾É?ÆYb`·Â?ÈÖ¯¸Ü?ÆYb`·Â?à-›˜'¼?Ò5 ÊcU?ߤÈÎÝÀ‡?Ò5 ÊcU?æ†6\LJö?¶;]|[?Òó"Ggj?¶;]|[?Ù®ÅÚY6?½µœ¬1ø?ã(Ótå?½µœ¬1øMIXED3FGL J1613.8+3410@KŽÀA¤@G,|?ìÀ9…'Uþ9VÀ;ۛárv?¿¯½_ïð7@.ƒíŠÝi@Кßê¶Ã¿è$¤ˆœ,'¿áÂÓþüR¿æÎPZ‹¿ÜÌñõ-xAGNfsrq@‹,¡aä÷PowerLawOS 319?ïú2ïýž?HïŒhñð?G4?ž¶˜?HïŒhñð?ïÏ@âj»,?ˆ¥ڕ­ê?x_ŽºÔ5ý?ˆ¥ڕ­ê?ïŸfw$Ç?€_<8Ýò…?ˆ&b3^£»?€_<8Ýò…?ïäÖ?WIŠÕ´çy?k)=|?WIŠÕ´çy?ï¼QŸ¯Þ*?…G|#8«?€ë˜ùñ­?…G|#8«?î"-DíÖï?·¾›Êøìx?¦Í+µn
?·¾›Êøìx?î&/@×­ô?¢þ&H)"˜?­ô<îÂ?¢þ&H)"˜?î5'Þê[©?¢›P™ê?¬¦ÒƐt?¢›P™êAGN3FGL J1614.5-2231@v	ÄupÅ@42«@‹
‹À8z½ø³oÀ;;…Ÿç't@Bv½K¥p@&©fÁ*,?ò˜(Ë{>?™È—«OF¿ÅPVHzÜÚ¿å³ìí\[Ü°×PSRPSR@–™xºÇËPLExpCutoffPSR J1614-2230?LÑQuààÇ?T[ܛ#?ïøË«V?T[ܛ#?¯™©‡=ð}?¸]v—Ö»?îegbå¨?¸]v—Ö»?¬ó'8›4Ì? 3tÿ3æÝ?î0ÆÜ?Rô? 3tÿ3æÝ?'gçcߟú?w'N°
æ?ïtÀÅ
>P?w'N°
æ?_UNqÃ2å?\O'otô?ïðUY	æ?\O'otô?¢ž%.2¤_?´£Gý¸÷?îÖ­SÏz?´£Gý¸÷?¢~ø‰3º?žÒW‡B­c?îØw=ñu?žÒW‡B­c?`«*dÿE\?R·gçA+'?ïïTÕ«~Û?R·gçA+'PSR3FGL J1615.3-5146e@tº£3v¿å‰€5´1À6ï¸GʐÀ9»–~\&r?ï$&O­@þ°³¼…'?ýÔ]àZô?ïýßÉÿ'ó?"¬'ßZö¿à'7'߿ހ¡{j×OTHERspp@·'=BÃÉïPowerLaw?çcCæM–%?Ì93ÌÏëª?Ñ9x3dÓ·?Ì93ÌÏëª?î£Û*ÍM?»*"[}1ã?¯åÂK›]4?»*"[}1ã?ãZ¹n˜†l?µ.
Þdß?ÙJ"Îó)?µ.
Þdß?íÙ¤•úS?š5nCKüz?±2ßzRì?š5nCKüz?é'yõíà÷?Å•ÆêúN?Éö(H|#?Å•ÆêúN?æªaÆw%Ú?Í搴(ø-?Ò«<s´L?Í搴(ø-?è-È»H?²œ®[çj/?ϓHÝ–á?²œ®[çj/?èÃÐûÁ¾?º…07øŒ;?Ìð¼ùÏ?º…07øŒ;AGN3FGL J1615.8+4712@RwïÝëÙ@FË/¿á+ÿÀ:X¤ï81 À;ìGJAl²¿Ë•ÌŸDB>@@q@)ªo÷µ?ïÙÖɔ£¿áòT"¿ÜÚòaSN~¿å=†uûYÓAGNfsrq@¤¹$Âø7µPowerLawTXS 1614+473?ïÿLÔo—?ç—ÒW{è?emòól?ç—ÒW{è?ïÁ!A‡ùx?¨"ž¢ÒYR?o_Xßûã?¨"ž¢ÒYR?ïÙåz `%?rcýjÎNÞ?s
BÕùt?rcýjÎNÞ?ïôõq p?A"T'g%?V-\Ê?A"T'g%?ïþ/©CŽS?2UåD´U?-hR%o?2UåD´U?î…ö·à_.?´¬šŽàMË?§ ""Â?´¬šŽàMË?ï¤ÓiҊ/?…|;øš)8?†Ë%™äE?…|;øš)8?﨏Ïo?|{LU±Ëß?…ÜF9".?|{LU±ËßAGN3FGL J1616.2-5054e@tÅـo&)¿ÀÈßK³À6"`4óþÀ9ákÀB{?·ä»uÊM@ÖSI3¦@(ˆ!ö¿áí¢F¼¿æ‰u_'®¿ãg–²^Œ}¿ÝÄ&¤`OTHERPWN@¥Kƒ¼ÓZ†PowerLawHESS J1616-508?ìR™Uà)?dz[tùYÑ?½k7uPþº?dz[tùYÑ?ïv­úà‰?©Jš³Ø²?'*@ xÞ?©Jš³Ø²?åÌöñ8'í?³ÊÜú'Ú?ÔfŽÜ&?³ÊÜú'Ú?ïüúZµ¿P?+÷%Ò[Žš?8-*ÛuÜü?+÷%Ò[Žš?îÛÉ+\ò?ª¦cS!ë+?¢Cnž&Ø?ª¦cS!ë+?ìwÈ]ž¹?Åꑳ
Ó?¼A½
7«?Åꑳ
Ó?ë9àAÚÒ?¯Å×]q
´?Ã~ø"·ï?¯Å×]q
´?ïïÎtö)Æ?TÕØJ®î?`1‹Ôùñ?TÕØJ®îAGN3FGL J1616.4+4631@R7Ã_Ñ ï@FÈûÿÀ? À:=aŠQþÀ;סS¢>"?Ù©¹‹Á-¡@­N€@­@»0à¿éaˆcÄÔ¿ê«ËŽå¿ä֌]é6²¿ïÿس"smAGNfsrq@…²ohیPowerLawMG4 J161600+4632?ïü½)ãö?F̺Žæ5?:¯Øœ?F̺Žæ5?ïÈVH6$ª?ˆR\+?—ò?{ÔÛÎ@??ˆR\+?—ò?ï™Pí/T?ƒÂ}?‰«ýršè?ƒÂ}?ï¨Ï	?pñL…(I?
æÎ"è?pñL…(I?ïþµh¾@©?4A&3úÄç?$©pð"å^?4A&3úÄç?í 2"ËÏ?Ám²q=E?¶þoÌG•?Ám²q=E?ï_M,}a?'d¼Ë«m4?"]½ßïË?'d¼Ë«m4?ë[èQɲw?®©•:9aË?^¸Ù6#?®©•:9aËAGN3FGL J1616.8+4111@PP9ßõž}@F÷¹¿©Î›À:"~êÁªZÀ<o%QÉ ?Ùf¯"ù>@Ù§b/'@ ™`
Ü·¿ã—"%ĵ§¿âP'gñ׿移*'¾¿ïÿWZýAGNbll@"Ðÿ—$tPowerLawB3 1615+412?ì¢`×J?Ò©=ÝAuQ?¿zìùE¯??Ò©=ÝAuQ?ï•fÏËbr?šä"	N?Š¦LåÓg?šä"	N?î/IÙÑ{?–ÓT©º?­boòèQ?–ÓT©º?Ia€?ˆ2|6ÙÇ6?¦F+n©è?ˆ2|6ÙÇ6?ã¦9s`—?ÕGËi(P?سÍ>Ò?ÕGËi(P?êe/NæÝ?ÉÚG¡K·?ÆjBÄd?ÉÚG¡K·?ꆮO»?³Çq	«Æ?ǝåG†Á?³Çq	«Æ?ãv² ?¼þl0Ï?Ùïš¿çë?¼þl0ÏAGN3FGL J1616.8-2300@v	é€,
J@3w›ßÄ÷À9¼6YX`êÀ;73Ëßg?ìN¼9'Ùó@:zÅnÇ@Ûÿo·H?ïŠ3•XÂ9¿çŠ"ƒÉy¿Å7&‡ÔQ¿ïÿæPlOTHERglc@¤û¯ÅoPowerLawM80?ï™]ŽrìS?šHpõ$Ã?‰¨œm"¿+?šHpõ$Ã?ìÔíßÛ·?¹û[7€—7?¹_è"&ãÅ?¹û[7€—7?éš[—;¬?®àßÏ?ɖ'£MÁ?®àßÏ?ë¶9‰¨N­?¦Xù'­?Á'Ù^ÅL?¦Xù'­?î¦éÁØ°Ž?­ÔI]‹P?¥'cä,Å?­ÔI]‹P?äˆF	œw?Ð
6ãµ?ÖïsìÇû?Ð
6ãµ?åß"j8-?¸¢ôôû?ÔA»+¥Ð?¸¢ôôû?ä-`3؅Ï?—šñˆmø?×¥?˜Nôb?—šñˆmøAGN3FGL J1617.3-2519@uî{¿"ÿ&@1Î9ßõž}À9(>Œ,ɍÀ;ç½f?ïÜÙ¤ƒ@
Þô¾@¹³ ©BÚ¿ã¥æÞ4Âï¿ê³'ɮƿåOI¥v®¿ïß²Ej æAGNbcu@'磢œwšPowerLawPMN J1617-2537?éQ4?ø"z?Ä@<±P?Ê»/²?Ä@<±P?âÈM>Õ±?˒k‡¸pŸ?Ûàoe'T?˒k‡¸pŸ?ê/"áaëi?¯¾šÂÔõg?ÇAìzxR]?¯¾šÂÔõg?ã'Ϻ‰~?ª‰PAÔI?ØÜaðŠí?ª‰PAÔI?â÷¤úuÒj?ÌP%¢Å?Ú¶[,?ÌP%¢Å?Ä?ó2ð Å?Çl'¥Ñ­ª?êð3C×Ï?Çl'¥Ñ­ª?ãqºGd­?¸²Hw)Œ?Ù‹q7Ч?¸²Hw)Œ?½,ÓG»+?¢†o'¬aë?ì]ºe—›?¢†o'¬aëMIXED3FGL J1617.4-5846@tp/hیÀ'ò€¯ËÀ8pº¼ÿÐ/À;I]A#·?Þª¶þÀv@n'!€-b@Þæ …Üx¿å÷ŽÔ'É¿èb¤‰ýè¿æ¶òI¿ï"äå-§êAGNfsrq@€‰W>«6zPowerLawMRC 1613-586?ïìÌ	êu»?_à$oÚY,?c3ö$Ã?_à$oÚY,?ï_áÍÃu?¡o vw?"#Â×õX?¡o vw?îèJ6"÷K?'©¡âXô:?¡{\› 'I?'©¡âXô:?ï¸Íegґ?d¤ç"¡Îf?Ì¦µ™­?d¤ç"¡Îf?ïÒ¢îƶw?u¾ß­†×¼?v®ˆ¢Ôp?u¾ß­†×¼?ëÌK/Ş?ÃFï4£>?ÀÎÓ«@éˆ?ÃFï4£>?íò¾
^ ?¡Ê·rî@,?°j¬Ò?¡Ê·rî@,?î~ßüKã?›D()èýG?¯è;AÓ?›D()èýGAGN3FGL J1617.7-7717@s–¿šÏúÀ2Ûú Âî'À8ª$[ÿÛÀ;b!¯é?÷whlP
Y@m¼Æð?@LŒX¦¿âËo2F¿çFMqj,¿ëϋó¿íA1×8AGNfsrq@yÀ=Ć­.LogParabolaPKS 1610-77?ï†3cK¶?‰@˜sNà?Žs'#ŒJq?‰@˜sNà?ïCl/—áø?ž#ïC?—'zKòú?ž#ïC?î0×'2Ž?"+!ÆîS?¦,òŒ×%?"+!ÆîS?îZ™ òÌ?‹ßzk¯e?®zVeìF?‹ßzk¯e?ïvTÙSÌc?…}7K6X?'5dՆs'?…}7K6X?éS+	‹?ÇPü$†Ð?ʳSáËÙÕ?ÇPü$†Ð?D¥]?šÉ¸ËW¬?¥TÛ²?n/?šÉ¸ËW¬?èýȺ×?µc¡Œ*å?Ïøݼ¢?µc¡Œ*åAGN3FGL J1617.8+5137@Sûݿη‰@F>'_ÀYøÀ9ÈÉu)wÉÀ;ýåÑ÷?åÏòª""B@‰Ð2
@—'ÀŽP¿æˆAÁ!¿é¿˜ð°¿ïÛÛ3©
?ékpˆB AGNfsrq@yû®]á\§PowerLawTXS 1616+517?ïÿØÙÝ>ýà\mqŸÄ>óûœ§Žò">ýà\mqŸÄ?ïÎõŒ€ú?'©až¨&?xôB®?'©až¨&?ï³Oo†~?ƒš`ó¯?ƒ,:—g҃?ƒš`ó¯?ïÿŸ	Åüy?ÒØì{ç?=™-Óð‡?ÒØì{ç?ïÿ¡c›
–?TÀS¦²V?§
3Ûµ?TÀS¦²V?îå³j	¼?°¾bš·£[?¡¤Éb/;?°¾bš·£[?ïb	­ÜOT?à~IJæ?"¾ÊB¾Gw?à~IJæ?ïùŠÉ®E‰?^ûfúž4?IÔ؎¾Ë‹?^ûfúž4AGN3FGL J1620.8-4928@tÞUùµc?Ø°ä_¡·\À6o'£+ÓÀ9·i$†È@þÊéG×°@
*Õô"»3?ÿ´>%–c¿Íóê:zG¿ß7åKÁ¿âƲ†@¿ëÈMt…–‹PSRPSR@™*øºÇËPLExpCutoffPSR J1620-4927?0õ€K‹{Y?5±p3)Û?ïýáOÄA?5±p3)Û?¥7ea¢•?Á"-Ô¤‡‰?©ó•?Á"-Ô¤‡‰?–ðô²4"?•§g9Trd?ïO¸xh,Ë?•§g9Trd?iIOø6m/?U	¬þ›Ž?ï涯÷Ks?U	¬þ›Ž?=n¤˜;?4Îe
:¯?ïü\Ò
p¿?4Îe
:¯?'>þ݆ÿq?¤ÿ2Æ=öâ?ï·‹CÚ?¤ÿ2Æ=öâ?~øÑ>ÌÆy?€Û–}Ö%®?ïÂ]Ä^ó?€Û–}Ö%®?=¯ÝÜÂk÷?5kÐ?ïüJtș?5kÐPSR3FGL J1621.1-2331@v'Àa"@2fþ?5ŸõÀ9*Et~WÀ;+Ÿé>ó[?úxÏ>ìúÀ@:Lj'Ä8@¥e;C"¿Þ¶a$vñ"¿éÆ»£"©ó¿ì¸ï6übß¿ÞÒ¶õä·êAGNagn@ë÷ÎÙ‡LogParabolaPKS 1617-235?êÿkœ‡½?ƁžÓ6À©?ÄQ¥á?ƁžÓ6À©?Ü/–³,µ?Ñ_[ßhŸ•?áè4¦i¥z?Ñ_[ßhŸ•?éðñ'ŸœŠ?°uÈüÊ?È<9¹×?°uÈüÊ?ã#ô'ã
›?¶cÙ$sþ?Ù¸ú9äË?¶cÙ$sþ?è­Ü1CÄÑ?ÉfFè¿?ÍH:ðì½?ÉfFè¿?¼7æB·+?ÂbõMt}?ìy7©Û?ÂbõMt}?èþ°;5yù?±£éÛy®…?Ì?*?±£éÛy®…?š®Ú;?·()ð¸f?ëYTIz¿±?·()ð¸fMIXED3FGL J1622.9-0312@%"¿ª¥[@>¶ÌŸóPÀ9PAÌS*IÀ;cÊõ\8?ê ¨ÍFÍÍ@
Ãt±­·‰@ß@QSÛ¿Éxà^*X¿æ4ˆ1ߘy¿Ýx(ïý\¿ìâ.w¦nƒPSRpsr@"0På`A‰PowerLawPSR J1622-03?ì¢t¬zFî?¸qb`äó?ºìZœ-Ȑ?¸qb`äó?íd
—?º"{q²Â,?³"ß™¯ÉD?º"{q²Â,?êÂnjtpž?­	_i
õ@?ÄöFV.=‰?­	_i
õ@?ê9Ižô;@?¢"•Vq"Z?Çل/?¢"•Vq"Z?è\ào…¹?Å=zŠq?ϲŒ~Aé?Å=zŠq?äãlޜûE?Ò=tlZé}?Ö9&BÆ	u?Ò=tlZé}?æQ_-·ô#?¼Þ¢<^w?Ó]A¤»?¼Þ¢<^w?×ݞúŠ'ê?º-O)Å–?ä0'ºì?º-O)Å–MIXED3FGL J1625.0+5651@U¦J`"@EÿÝÑÀ:•é ÀièÀ<­2ӑ㿷@X»§S@"x´q·'@+¾aO?ïýØ¢1Ýb¿ê«»ú¹çd¿àgªÝtöÞ¿ç³Îߪ'ºAGNbll@'æ/·éùPowerLawSBS 1623+569?ïpHë‰Ùç?À1‡õµ×Æ?'ö≝Y4?À1‡õµ×Æ?ïÖlWädæ?}Tߤ¢?tÉÔ':¨²?}Tߤ¢?ï\×0u`!?ŽÍֆ5Ãï?"eíä_ì?ŽÍֆ5Ãï?ïÊ2ßXô?cF¤A¤ÎI?zæ]$Ý&?cF¤A¤ÎI?ïïŸ6Ö?"•^úËÞq?`ÿãŒÄ)~?"•^úËÞq?îwŸÿ?´ˆ â;?¨†nÐÃ?´ˆ â;?î"Ô¥MÕ?¢¸Ñ[;ŠÒ?­ÒµªRk¶?¢¸Ñ[;ŠÒ?íÃÌ©Í‹?£^՞8¬ó?±áš²ÝÞ#?£^՞8¬óAGN3FGL J1625.7-2527@vP +"@0Ri¿·:"À6ñ\°Úþ¿À:u6xbm@O( °z@ðõ£ÒM@ÑBG£,À¿ßVàßØ¿å!¥øÞ´½¿æKf©¾f¿è«ÁYŸðAGNfsrq@‡š,1&éLogParabolaPKS 1622-253?ïùfÿú‡×?[ƒ¯@ڙŸ?Jd³?[ƒ¯@ڙŸ?ï•y¯¡÷??¥œœ½ÂA?Š¡"'0O?¥œœ½ÂA?ê} ¸9öO?±½T•Ë²/?Æ}&Æ?±½T•Ë²/?ï՟žÁ—?`úýJ®ú?u00²?üÇ?`úýJ®ú?ïÌô÷}k?|5ÏÙ?y…"5Ǟ£?|5ÏÙ?íý"׊.Ü?Á¤º¿¯?°éC®‰?Á¤º¿¯?ì'ûþœ0U?ªFI]àê?»h }U?ªFI]àê?ïÑXæÝ*y?q­SÒé[?wSŒ—š\?q­SÒé[AGN3FGL J1625.9+4125@Pa¾À//˜@F@`B_÷À9Õ¢"›À;Îï@4£¿Ïk¶g/º@'G¡)Zí@›ŠË<T¿äoG¬DŸ ¿éÔìò9Ì]¿â›i+Mò¸¿ïùÿ•¡èHAGNfsrq@思IRPowerLawB3 1624+414?ïý±/§&d?,UŸßœ?2v'ŠSÁv?,UŸßœ?ïÑh­4ùS?‡Ò"ǃ¡?wK©6*?‡Ò"ǃ¡?ïÂFY‰;Ü?g)®d1¤?~ÜÓ1>
?g)®d1¤?ïèò¸bÝ?P›†Ñ¼Zð?g
æäòð?P›†Ñ¼Zð?ïý"–Ë3?3Å÷=(j©?3cGàN?3Å÷=(j©?î–)'Ì?²dq×ç:À?¦m‹4+J?²dq×ç:À?ïʦÐA?|¬^nx?z¬—ø­™â?|¬^nx?îÛª,±0\?"‰uÍ-+?¢E]6¤ÈE?"‰uÍ-+AGN3FGL J1626.0-2951@uÌó S\ž@*¢:Þù;À8>þ½	á*À:×Eßaô?÷¦g½ÿT‰@ Wš»-@IA½d¤ð¿ÜÕäÎ _¿è' +ø	¿äˆ=H,a¿ï	â.*W9AGNFSRQ@P{çl‹DLogParabolaPKS 1622-29?ï»5ɼ€?€&?(
À`?2¿@'\'?€&?(
À`?æXndÊ'?Æû«Æ®?ÓO#6ÄjÜ?Æû«Æ®?ëûç¬÷ð<?§a_Ga‰?ÀaL ??§a_Ga‰?ç%ê»ÓM?¦Àu¿^u?Ñ´+òˆYg?¦Àu¿^u?I¨üŸ?«Ç°~ôí?¤–[bš?«Ç°~ôí?Ó¦Ñ`/j§?ο5×ʤ ?æ,—OèJ­?ο5×ʤ ?êñᮨ–Ú?°"DZ38?Ä8yE]¤˜?°"DZ38?ԊæÆѓº?¶#oç[¨Ï?庌œ—6#?¶#oç[¨ÏMIXED3FGL J1626.1+3512@Lr"_õI@EôŸëWÒÀ:ۃ6€ÅÀ;ôyŽaW3¿èb‡Žv8@|¼êº?û2ýáAÎ׿ïÿ2Ìʸ9?ïýíXTø!¿Âs,·1ô´¿àÅÙ=žqAGNbll@¸Ä²@·€4PowerLawRGB J1626+352?ïþÕ±Þðø?‰-6B˜V?"¤ã	mÚ8?‰-6B˜V?ï¼Èy<=.?­[z/^ ù?€Íá¦ùÖ}?­[z/^ ù?ïÃÍDkêµ?|'D9Û6?~]êVùt?|'D9Û6?ïý©|CP?$¼ì
?2´Ùg"ß?$¼ì
?ïý†Iõ[P?2+*_ò>Ê?3ͲCí<D?2+*_ò>Ê?ïpîÓ?ªõÏæD´?1â/m?ªõÏæD´?ï'ï…x>?‹+"Ž7u>?{"(ðÄa?‹+"Ž7u>?ïêËRÌV?d
'dô¡R?e4­®9éÐ?d
'dô¡RAGN3FGL J1626.4-7640@s¤*ÿójÆÀ2Î_¿ƒ8.À9ÜKŸ:ÃJÀ;'"e'¿ùS)ÃGèÍ@+è«ûpú?ÿØJ^Èã3¿éI4'ª-¿ÔNd8Üü¿â‹&9O­¿×òÕÒ|["AGNbcu@¬ú;~ÿ—PowerLawPKS 1619-765?ïýµ9!"©?0i"»Ê?2V8#aL?0i"»Ê?ï·j;k?•C¦\›mv?'%qB|@1?•C¦\›mv?ïã&8MF?jšr=ß[?lÙè¨R[?jšr=ß[?ïÿïu²ùV>ÞUq¥d>àŠ‡põ>ÞUq¥d?ïúÀºèJ?@?{̽s7?Dý5xT?@?{̽s7?—<
?¶ê'G|?§å6÷/?¶ê'G|?ïΡdOq?z¤ÞþÉæ;?x¯M¹ZúÙ?z¤ÞþÉæ;?ïþ'‰Tˆ?'À'¶q?'×mÕB¸?'À'¶qAGN3FGL J1628.0-3203@u·(€QÉ÷@'½ ‡_À9"éû±¼¦À;<êºô]5?û"á·©°@a&xº¦Ú?û ¤†_¿ÀñÒQ{Y¿Þ‹·½"k¿ë"Ú±¿ïÿexª¶¢PSRpsr@FE8ï4×LogParabolaPSR J1628-3205?±Ü	øô•?¸a¦y Ë?íßd~|)>?¸a¦y Ë?°Ô0VO'?ºé7;«|Æ?íåyõmž?ºé7;«|Æ?Í'|Oíå?±)ÉT>½ø?踛 ì‡?±)ÉT>½ø?ÁԫύW¨?¸ôE=[?ëŠÕª?¸ôE=[?hmJòqÀð?nSÚãÕ?ï璵=¨Ç?nSÚãÕ?–²âò§Gš?«áKH£"á?ïJhè]S?«áKH£"á?¡6˜+P'ð?™K\zÀ–?îì–}t8Ñ?™K\zÀ–?‡"6åP?t¦à>mÃ?ï£w$4ùÃ?t¦à>mÃPSR3FGL J1628.2+7703@[×6&-@A(?º*3À:†±Ö§A"À<bf&¥†À‹@€MÃ,@Í¡²—ÂT@—Á_±@¿áàð|¬,¿ç`Çk¿åšãˆG"¿â3 C+ù®AGNbcu@Œ%/ƒ{J#PowerLaw6C B163030.4+771303?ïþzµ0†?=ýa+j'j?(T¬Ëì¥J?=ýa+j'j?ïä˜÷:è?~åa¦à•\?kgË÷&ø?~åa¦à•\?ïÅ–õzk?v$p°ÞZ?}t4n•^Ÿ?v$p°ÞZ?ïÿþ'í'û>¥³1)s_4>¦Ðù×KuÈ>¥³1)s_4?ïõ·¿@êx?a-‡¿%ì?Tb®/…?a-‡¿%ì?ïN·Ø–Q? ¿.¿8ú?–)ë~? ¿.¿8ú?ï'Þ«=þ5?—|ÆTV§(?›*©3s?—|ÆTV§(?ïÿ¸t[®?	Ԑ2ω?ùaa§zÊ?	Ԑ2ωAGN3FGL J1628.9-4852@tô	`0Â@¿Â±Ð ƒÀ8#ÙìpCÀ9ð¿UK?ø/L>h@ÝéÀ"š_?ùw/É~?ïù•‹–¢¿â3,}6¿ç…sq礿îA¼}Ê0:OTHERspp@ßŽ_oÒLogParabola?dƒ%ÙÂJ[?vQõø^…Ð?ïë|Ú_÷%?vQõø^…Ð?½‹H]'Ö'?ÁžÊ}^œæ?ìN–ôMÅ0?ÁžÊ}^œæ?ÄǨž?«ÏÿKä«?êÎø˜`<?«ÏÿKä«?ÔÒì:j"ø?¯ÂÓ(ûY¥?喉âÊî"?¯ÂÓ(ûY¥?F;¥ÏEÖ?O_z‹š÷5?ïúq²bØ?O_z‹š÷5?˜üqŸq¿?« fN~î<?ï8rì'?« fN~î<?¦ÌÚ!"½K? ì‡crQ?î"2^ï{? ì‡crQ?°~AÁ+Þõ?šj_C¡?íð7DZHÒ?šj_C¡PSR3FGL J1630.2+3733@NŸ C×Æ@E¥IÿþRÀ9´ s¨nIÀ;Ÿ0¡ˆ{d?úxuz*"|@©°Û.d?ôÅ›À?Þ,ôæØwâ¿Ü£9~Y׿àl³Ã¢'οïÿëÙ¾ˆøPSRPSR@˜ÿq&éxÕPLExpCutoffPSR J1630+3734?¹ƒÔ³°x?ºÜ´ì}?ìϟ¥wHa?ºÜ´ì}?Ï+øÊ_<Ú?Ò"ûÞïJa?è5Íh0É?Ò"ûÞïJa?ÉÚÓB)<²?±G!¸oD?é‰K/u°Ô?±G!¸oD?Í ¾ò¶°?©~b" C?è—ÐCyÒT?©~b" C?šës5i´É?¢'4ÔCî?ï(¤f¸š?¢'4ÔCî?½ãDY1…Å?ÉÖ°™nF?ìC—tÙÏG?ÉÖ°™nF?¶a2ÙäL?¬ªð¢Vc?í3Ù¥žÆ?¬ªð¢Vc?¥Kù¥3[?"YÇ"?î®k@sk:?"YÇ"PSR3FGL J1630.6+8232@\ó(^ÃÚ¶@?@*@EjmÀ9<¿"ÀiÀ;¹½îãx
?ö*6ÊÂ[…@I¬3$E?þ9[-£&`¿ÒmOÄcq¿¿å¶3ƒ:2¿ä|1Ën™¿çÜŒ{›AGNrdg@ˆH´¢3œLogParabolaNGC 6251?í°ºÏZ'?²¶4h¢?²{'*að?²¶4h¢?âØ]7RÊ?Ë<ÓèAj?ÚOE'ÉZk?Ë<ÓèAj?íy–ç/?§FƘ=>ž?·ì3G¹*?§FƘ=>ž?ãÙ8$"ã?¥]éB¹?ØM·ºä9?¥]éB¹?åi¯lÐÉî?È8Ï\ý–?Õ,¡&^l%?È8Ï\ý–?ɲ³›ùEQ?ÇG±‰>?é"S®¬?ÇG±‰>?æ+Ë(™'?¸£bδáý?Ó¨i®ÍæÜ?¸£bδáý?ÃÅ>M˜.?£pŠÿ
kí?ë°l™Ü5?£pŠÿ
kíMIXED3FGL J1630.7+5222@TÒÿ" @E2_×ÖìÀ9?¡F6E6À;'úÀûÞ2?àáøÆ®XK@'uiŽŽú?ÿæü9¢¿àí7[¿w¿Ú#{£¬\¿á¬ž=1'¯¿ß6"›¹ë…AGNbll@œjöý!ÿ.PowerLawTXS 1629+524?ïþeï{«û?#n-ªû­Ñ?)¡ö¢?#n-ªû­Ñ?ï×
)M)?›vŒ?tykDÕCª?›vŒ?ïäþŽ:ì?rsĤ,š?kä¡ßœ?rsĤ,š?ïË5¬En?]\Ø/ÅØ?zexCJdù?]\Ø/ÅØ?ïü"#Q¤ô??ï…p‹ñ?>î㉏þÁ??ï…p‹ñ?0É?²8C§n†?¥¥,ÿVô?²8C§n†?︧›‡Qæ?"%'¶a(J?Öm¡?"%'¶a(J?îìuî¥?•Ü{³®€?§á8²¬˜­?•Ü{³®€AGN3FGL J1630.8+1047@:uxmži@B/ÿ¢/À9›ÉØ)øÀ;†™°?ÎL?ár'3Ô÷F@éFÅâ!ô@o¬ÙO¿â"¬5[47¿íÕ=}µ¿â6}g߸7¿åÙEìüË¡AGNbcu@x¨Ÿ¾vÉPowerLawMG1 J163119+1051?ïþf•`Nõ?0öWÒ#IÃ?)–ªS¬|?0öWÒ#IÃ?ïfçÅ÷p?´µçuH=?"#8zè ?´µçuH=?ïÁ­ú?zWȾ@e?@)yÀî?zWȾ@e?ïî$,Òh?ø/ÜN?œ";s†zý?ø/ÜN?ïùIÓÏW?PíEÒjñ?JØ´ñý+?PíEÒjñ?볖C-
?Â÷˜2;fˆ?Á1§þóKÎ?Â÷˜2;fˆ?îðчOGÄ?—M‡4v±? òçŒÃQ·?—M‡4v±?鄕@n…?±í"È<¨?ÉíªþEë?±í"È<¨AGN3FGL J1632.4-4820@uŸà·ö¿ÉA×ép-À8Bî'sÀ9æŸÐë??ø‹9L&õ@<öùñóù?ø5^ɹòÕ¿íù"ýW`?Óø/ª´ì¿åJ#ËÈQ#¿ê4zý2nPSRpsr@¢N.záHLogParabolaPSR J1632-4818?D€
ZŸF?ŒO¾W‰Â?ïÁw	±?ŒO¾W‰Â?Ö©0
3à'?ÎV0G_Sç?ä«gúæ¿?ÎV0G_Sç?Óq/îTù?´Šƒà7ñ?æGhýՃ?´Šƒà7ñ?á¼Ê¡#|?²À
v¶Ï?ÝІj½¹	?²À
v¶Ï?"@œ[J"t?¶Câjß@?ï®ýŽ¶'¢?¶Câjß@?«—éÑvqû?·"ÉZd?îFbÚÚp?·"ÉZd?ºÇ?bI(ñ?±B1Í´Q¡?짶Úâ?±B1Í´Q¡?ÃE›Þ èK?®]KtB~?ë.™WÅí?®]KtB~MIXED3FGL J1633.0-4746e@uGñQç?¾ó@`å•hÀ6°\S½íÀ9aÓÚÞ?ç	÷¹EÃ@ì!´@â¯3+¦?¿§¾åi¿ãg´¯Ÿ•\¿ãvt€Û\³¿ã†.þE?ÐOTHERPWN@§EoPowerLawHESS J1632-478?ê|&'±?ÍX¼¶':?Ægcé<?ÍX¼¶':?îúÀI vÇ?´®Ô7{ø? Sûe¬Œ?´®Ô7{ø?â»Þ|ïâ?µ5='€&?ڈC ;Æ?µ5='€&?îö}C?ŽÂ‰Ù±Wi? ˜._ŽÛÐ?ŽÂ‰Ù±Wi?íÙ÷Yà"v?µ~ÑÂ*?±0E2³2Q?µ~ÑÂ*?éC\+Ë­?Ê=Ž1lÅ·?Êò÷PÑK?Ê=Ž1lÅ·?éˆem~Cä?²F"@¾?ÉÞjJðp?²F"@¾?êE1Ú»?³êìï€K­?Å¿†ë8•?³êìï€K­AGN3FGL J1635.2+3809@NŽ?é$@E+uÞÝqÀ6°"T"—À:¬Ò['@ä–ü±A@z®ž@©š¶$>Ï¿á\¿Uڗ¿æۋV`Ë¿çË,æÃ¿ë+ômáÁAGNFSRQ@…é‡?úÁÓLogParabola4C +38.41?ïÑèރâ?zÝç»áN+?wÄî8?zÝç»áN+?ïÁ;zù?¨Œ‹nQ¥?rât£›É?¨Œ‹nQ¥?ë
'AOon?¯Rü:lÃ?ÃÕ¶úÂBI?¯Rü:lÃ?ïõRx®ùŽ?E™'ÈÂÙ?U[ƒÐSp?E™'ÈÂÙ?ï"Ë?ó¤Â?õÌ´ôË?‹
0
e£†?õÌ´ôË?îœGcÁÆ^?¶xµ!àP?¦;‰Ã³?¶xµ!àP?얰Äa!?§­=+ØÁ?»JyÜö÷ª?§­=+ØÁ?ïøkXŠýí?Nlet•?NRžÕÞ.š?Nlet•AGN3FGL J1636.2-4709c@ubŸœèÙ?ÀèÏÀOÄlÀ7f×süPÀ9‡ëÕ¦"?ô"Þ+ÄÔÜ@4ýOü@·˜?§_Ö¿çñ¡B…a¿å©î{s>¿ç¢8¤Œ;ã¿èW}?pÙ1OTHERspp@«/MúCþ]PowerLawt?°>4'Á®Ã?·tðbJš?íø9mñw?·tðbJš?å²Î²¼;–?DŽI!c?Ԛbš‡ˆÔ?DŽI!c?ÑÉ&vٝ?µõ
^3Ú&?çlē19?µõ
^3Ú&?çjEË&§?¦ü§æü]e?Ñ+täi²²?¦ü§æü]e? ý€­f4z?¦Éێƒ&k?îð'õai?¦Éێƒ&k?¼$›ž_.Â?»~¯)ñ•?ì{lŒ4(?»~¯)ñ•?ÐÏ$–ô^ó?¸¶vþé~?ç˜m´…І?¸¶vþé~?ÏÕz¡Âï?°áMžíŒ"?è
¡WD<?°áMžíŒ"MIXED3FGL J1636.2-4734@u{à~í¿ÄC€³CºÀ6ä'eîqbÀ9'!àÄÑ@=ÃòI´@ž>ïÔå?ûC¼˜L=?­Müƒ"À¿â8¶)ó'¿ãþÒ–³5¿ìö( ­9OTHERsnr@¡5?|îLogParabolaSNR G337.0-00.1@?4'A©½‡?72ÊëÐH?ïý{šÈ»?72ÊëÐH?£Ÿ¹³ßMÕ?¿Ÿä-Þ×ß?îÆdÏɓ?¿Ÿä-Þ×ß?ˆM¢"?=IwóJž?ïžÊZ6ò?=IwóJž?Ÿ.E+»í?ƒ±G­ã'?ïÖË[ç?ƒ±G­ã'?7¸ê· Ñ?/Ÿ©9Zûµ?ïýâ°A"?/Ÿ©9Zûµ?ŠËIŸCBC?ªò^Àuhœ?ï"ÒÙgv?ªò^Àuhœ?{_í)O`ç?}EH

%ª?ïÉ@%èz†?}EH

%ª?wW},ŠÿK?j}ë–þ?ïÑQ׉?j}ë–þPSR3FGL J1636.7+2624@Fßß´0@D€C‡>À:FوœòÀ;Ú´*>—ë?áfà•'µ
@ñ‡î'ð@Pbà?êøì#eq¿âÅAµ?¿×-ɀ«Ñ¿ãÊ*î7¢üAGNbcu@£l IQƒPowerLawNVSS J163651+262657?ïýïg•&?1@×}fl?0"Ê4D¨?1@×}fl?g¢{•?•"‰ªª?‰f!¯î"?•"‰ªª?ïÌ#ØÞd5?uLøçìè"?yî"•o?uLøçìè"?ï`!†k?'*ÇA±û?žö§È¤?'*ÇA±û?ïòl{ÿ)ì?[äK¦…ß?['x;ÈP?[äK¦…ß?ì©}ÝÈÀ?Á
"o¸?º·\º?Á
"o¸?ïc¤Ô
?ÑÙÕ]ß?"Ÿžf>¼?ÑÙÕ]ß?êº$"a'?±ö¸•_?Åo¹²yö?±ö¸•_AGN3FGL J1637.1+1314@=ÿ¥ßøù|@AÙÚÿ•võÀ:HNäi¡"À;›üD}Þ?ÇÇ9‹£@§ºu\M‰@Ä¿Àéz¿ì/죛"à¿è˜É:.Û¿ÃÐ'Ü}¿Ñħl¥ÎAGNbll@¢(ʦL/ƒPowerLaw1RXS J163717.1+131418?ïþAôÅ\?<í£&A?+îT¿g²+?<í£&A?ïÀ|'˜e´?*^
gÜ	?Á·#þñè?*^
gÜ	?ïÆÑ
I/?z¿ï¥²3?|—zô% à?z¿ï¥²3?ïí©Úô?MO±h³ÓR?bðV%äK?MO±h³ÓR?ïûD@:œx?GÖâRړ@?BîÿõÛ²?GÖâRړ@?îÿ9u*?¹Ôx×qi?®PlPßa?¹Ôx×qi?ïŒÚmì?ŠÍtg…ö?ŒÉdl£®?ŠÍtg…ö?ï|ˆø©?‰¤åÆüzÑ?nÿ€íêî?‰¤åÆüzÑAGN3FGL J1637.6-3449@u«•¿ðEx@ \îøœÀ9Qc"GÁÀ;"g¨…ŧ?ñWmû@
a–4à2?û¶¡>ÿo6¿ïÿ¿Ä.KK?ïÿ†ªBx¿ÛÓT"	•^¿Ò4>ñ'cÈAGNbcu@¸0íÒñ©üPowerLawNVSS J163750-344915?ïمAóÀ? göIÍó?œ¤ÏTQëú? göIÍó?ìtÅãQ§?½œeY~ª?¼Y×ÈårÇ?½œeY~ª?îŠ×Ö&x÷?™Ìx+?§R'›à¢–?™Ìx+?ì€Ã¼Ø¸é? ÌZ¼-%?»ùâ:8¶? ÌZ¼-%?î%Ø»(Ư?©$$NŠ®?­¢tJù?©$$NŠ®?Üôt`úì›?ÑH"üâǾ?á…Åς‰³?ÑH"üâǾ?ìÍ¢š@ªâ?¦õD^?¹'ë.֏ì?¦õD^?âMÉ-þ7u?»lmà>?Ûdm¤'?»lmà>MIXED3FGL J1637.7+4715@RYÉ`0Â@@DñCÀI0ËÀ8'滋[éÀ;ž{Àj¾»?äôÛìû@~@T7$Y{œ@ð°ÿç¬L¿ã{·¨<8"¿åæÞP$R¿ä
këØο谨Ýaø÷AGNfsrq@' çÀn¹PowerLaw4C +47.44?ïÿMyÊ52?˜:<[Ì?PĺL9?˜:<[Ì?ïÓ`[¤/d?‰iž·ã?vOÒKæg?‰iž·ã?ïçTïJd?iü­‹¤?h«<#ZÄ»?iü­‹¤?ïþð§dD?
V>5vý? ÿDÕißj?
V>5vý?ïÿS	'Où?(ƒqêÓ?žÇõ"Û?(ƒqêÓ?îñp¢]?­îËtŠ? èõßV?­îËtŠ?Vlb?€—¬ºÌ¯È?€;'klÉy?€—¬ºÌ¯È?ïýi7Q%?1:Ҝ?X?4¶C"(ö?1:Ҝ?XAGN3FGL J1637.8+7325@Z~V>Ðö'@Aœé	:;À:è¢[ßú§À<<zØä2D¿¬'–°OÄ@ºðëeU?þ™é`+cÜ¿í]èK‹ø$¿¾­èlK¾Ö¿³a»Fg˜k¿çòג<rAGNbll@°mý\ú¬ÚPowerLawRX J1637.9+7326?ïÒñ–¨?ŒŠ`Ò¹Üì?v‡4»Á0:?ŒŠ`Ò¹Üì?ïÓ¿¦"'?… 
E¸Ô?v ,¤ÝrG?… 
E¸Ô?îBՌ±K3?¢eç†#ª†?«Ò§8ZèÃ?¢eç†#ª†?ïÕë".?`¿9÷ª"f?u
~…­X²?`¿9÷ª"f?îåÙî‹ä?­‹ê·õ$?¡¢o_s½?­‹ê·õ$?î—xÉ?²$í/1?¦Ž|»¡Þ?²$í/1?íÑÚü÷s%?§û9]ùî4?±q( MØ?§û9]ùî4?ö˜?žrvZž]Ù?¥†/¼R£ˆ?žrvZž]ÙAGN3FGL J1637.9+5719@U¨s¿ë<ú@D2Áð8À9ÎØuw{À;÷–uŸÀ

å@CsõÆN@p¸ßÚñ~¿êýiEÛ_¿æU¢å®×*¿ëñð¿åžo"r@AGNfsrq@y)SeâXPowerLawOS 562?ïÿÏFàËC>ûj€Ãû4>ø\†z «>ûj€Ãû4?ïáäC€…?"$ƒE??n½4y:q?"$ƒE??ïÙ¾ìJ§ª?oÚ$'>]1?s ‰¼o›
?oÚ$'>]1?ïÿþ4 >ª,i>®KLޛ÷k>ª,i?ïÿ{£íãü?Ñï',²ª?‹‰y\¨?Ñï',²ª?ï(}}Ôö?«*ùÙÄX¿?šð^ÕÅR?«*ùÙÄX¿?ï¶Ì×é?û×6"&?'zŒ¼ÓÖ?û×6"&?ïÿÉ?é=à?'Y|>û_ñet¾?'Y|AGN3FGL J1638.6-4654@uƀ"?u©`À7W=¼ùðòÀ9¥ýò߆
?þp뽨@g¹X%ÛÝ?ü·2Ü¡+3?Ç1i™÷k¿Ý÷áìåLjar¶¬¿ê*r.ñ…OTHERspp@žû1[W>«LogParabola?¢ž
a#?«!ÞlÊh?îß6¨•>?«!ÞlÊh?¾	ÛçûZ?Á­‡Nà°&?ì>ÝDƒ•?Á­‡Nà°&?Ä«J%èòÈ?¯E^¿4%$?êÕ-v…ÃN?¯E^¿4%$?Ö¬bõÿ²9?¯¡â.é?ä©Î…&ä?¯¡â.é?§ØFÃ&éu?«n`ÂÎÌJ?î'{"ÛOÙ?«n`ÂÎÌJ?ŸT'U6ü?®‰(6ú ?ï[mN`?®‰(6ú ?ÑÖ»3Ù\Ž?·p´XÛ»?ç¢fQ¹?·p´XÛ»?½Wþ?qÁ?¨cög®mš?ìU8ÇÜ?¨cög®mšPSR3FGL J1639.8+4125@PdzøÞ¤@DÎ3_¨ÝÀ: ¸jßrÀ;ÃiÔ¯ð?à›{'=™@"NAxÆ@UÀâcb¿ãõ×|B	ª¿æϐnw¬à¿è¦˜!ˆˆ¿ïýžIè½AGNfsrq@‹Q=ÈKPowerLawMG4 J163918+4127?ïügVìB?8RòÇõÉ?<Çc±Ì/Š?8RòÇõÉ?†¯\?•ÂÓ¼ºŒØ?‡Þz!ÃÄò?•ÂÓ¼ºŒØ?ï¹H¿0?lWD>Ü$R?­ÐEšÄ]?lWD>Ü$R?ï
XúÜÄU?|ijó¿Ú;?žTàˆ=[?|ijó¿Ú;?ïûš²Eø?Aâ–ZK5?A•7÷–±Ì?Aâ–ZK5?ì_b"ÛÕå?Ãw
ú$Úç?½ëY!PÕ?Ãw
ú$Úç?ïœè揹?"ÌÒIÓ"?ˆÅü¼
=Ô?"ÌÒIÓ"?ç\&,PÛ?´ä*€iï?ÑG³Õ§^K?´ä*€iïAGN3FGL J1640.4-4634c@u$_•'Í¿"'‹Ÿ«¸rÀ8Ø{,ÇÀ9Ñ)‹ê"n¿ö0	£—Ê@
jthÏ?ý»¯ÞÕbó?ì} ⣣´¿â:Áœíáð¿âNªRNm¿Ô½p"ý°ðOTHERspp@É×®záPowerLaw ?äp%,'ã¦?Ѝ8WŠU"?×µ¦Ú8µ?Ѝ8WŠU"?ïœý)+?˜a–Î8?ˆÀµ¯}EK?˜a–Î8?ä'¨8ÿâ	?´XEU¦xñ?×°¯Ž;î?´XEU¦xñ?ïÿµ P?J×ʃ¬õ?¸{Ï®³?J×ʃ¬õ?ç"1÷㕫?Èíï>38ß?Ðל8Ôª?Èíï>38ß?íð\ÉÚ?ÂòwBùò?·X}û†?ÂòwBùò?ê@"òît'?°åìK6B?Æýì4F-·?°åìK6B?ïû@æؚ>?CúíÄ'n?Bücûö5z?CúíÄ'nAGN3FGL J1640.6+3945@O¬Xߕ&m@D²•ÿ±%§À8æ…Ûv´À:"+,Ôta?øãW/ç¤?@6€´yS@5­ƒCl¿ÐbÜXŒ¿å~¯´ý¼ó¿ãÝtŽ-î¿êY©1<8AGNFSRQ@"üí'hsLogParabolaNRAO 512?ï⋟þ/?m~™]EM?mt`În?m~™]EM?ï½G;RçY?–ËšÙÆÁ?€®1wõñ?–ËšÙÆÁ?éó·4Š U?®ÂMĎM?È1#-×~­?®ÂMĎM?ïÂ5o"¢—?bZp8ø,?~åHWQ\~?bZp8ø,?ï*ì<ãX? a¦€`LA?š¢Øc•? a¦€`LA?îyl}µø?µ°*áAÙ?¨i8*xUz?µ°*áAÙ?é=LÌ-âß?±Bì¢uÎH?Ë
ÌÏHt…?±Bì¢uÎH?ïÂ—-a?''ÛÎݝ?‹ÏZ1)Ë?''ÛÎݝAGN3FGL J1640.9+1142@<āŸ§Ð"@A–`)5ƒÀ:ÛeìÃãÀ;•ô©Š¨e¿âêz6Õn@Ív&wãç@]P¨¿äÌ®>0+¿æa†&(¿Ð­b…÷¿ëb$yµùAGNbcu@›-w1ÅPowerLawTXS 1638+118?ï󱒁ç?Y9/ä۟–?XœÚ«W",?Y9/ä۟–?ïÄÇîtE?"¤>,§?}ý›ñh…¡?"¤>,§?ï"ï̬?¨²¦#$?›®ýÓwX?¨²¦#$?ïöˆ;0??ôb	)àQ?RïÒ';·??ôb	)àQ?ïè}'ró?n0#	u™½?gñ'Œ«UI?n0#	u™½?îgt'òƒ?¶i¸Wª?©ˆ·*@sÍ?¶i¸Wª?îa®5vô?ž:­ˆ¶]Ð?©å+Ì©À?ž:­ˆ¶]Ð?…Ä?…Ÿ6·§@?‹ùèÝÑ6?…Ÿ6·§@AGN3FGL J1641.1-4619c@u(; îÙ?®æ»Ÿù'À7'œh€òÚÀ9›œÈù¶¿ÏcôçH#/@
ešO±™@:_¢Qú¿åPŸŠtb¨¿ë%nâO¿Úÿf}›¿æ|Í{Hu»OTHERspp@›}åÉäPowerLaw$?Ðæ…Òß­Ç?ϖáŽ$ñQ?猽)?ϖáŽ$ñQ?ïkìÙ÷F?ª'‡3\ñ?''d¸€(s?ª'‡3\ñ?ߢ2PExì?´—ÓâV¤?à.æ×ÝCŠ?´—ÓâV¤?ïàUw«¼?j³р~~?oªˆÊ×c°?j³р~~?Ýz«9L?Î]ãº=í»?áwþBªcZ?Î]ãº=í»?ëÌøŸÊœW?Å#W×òµ?ÀÌ€ÕŽ¤?Å#W×òµ?æHjxªòÄ?´ÛÜÖ4sˆ?Óo+ªy?´ÛÜÖ4sˆ?îÄU&@Ã?"=èÓD‰h?£º¯°/¨Ò?"=èÓD‰hMIXED3FGL J1641.8-0619@%¤rAeûÝ@9ÅYa›À8ÍÎ8׋À:æÃr°÷"ÀëýT©û@ˋo_^_@†î_ċ¶?ߟ'
ÈÊ£¿äeún#QÇ¿ãEk5œÞ·¿áÊÞ:ˆgAGNbll@šTɅðPowerLawTXS 1639-062?ïô™ø횫?Yjœ¯bT?VÌ«{X»?Yjœ¯bT?ïªmG3ÎÂ?ŸÓÿ
j5y?…d®%Mߊ?ŸÓÿ
j5y?ïuãÞ>î?Œ"/¤Ï?'_ã{¡V?Œ"/¤Ï?ïÿý"ê=>³1쪪ÿ>³`örÜ[>³1쪪ÿ?ïúm-ø-E?Vî¿D/Ñ?FKHVD«?Vî¿D/Ñ?íöœÿæ?¼dÏÀûã?°OۍôQ?¼dÏÀûã?îÉÌM‡-—?–Èû>̯Ì?£c;&±?Š?–Èû>̯Ì?ïÿÌ!ìÁ?ܟV>ùïŽì`Ö4?ܟVAGN3FGL J1642.9+3950@OÀÍ_™Ã‹@DyvÀP½ˆÀ8"è1­!À:Á͐A+C¿ôÁ}ÿ	_û@;64D€8@"H?ß¾í¿å֜ƒÑ'È¿åÃT±¹Õ¿æ0'êðñ'¿æ‹Z˜
8´AGNFSRQ@'ó¶E¡ËPowerLaw3C 345?ïÿŒZÊY‰?fÄB&»d?é[«š?fÄB&»d?ïÐä¾øØ?‹‹Õoý"?w Þ¥›ê?‹‹Õoý"?ﶼ/Vì?'DÒES?'yó"c?'DÒES?ïÿúZ¾VV>ÀmOªIÂ>ƕáï1>ÀmOªIÂ?ïþÆIzó;?$‡Ï™«‡¦?#›eÊIü?$‡Ï™«‡¦?R$B³?³Ó‡V?	¨?¤Tjá+pË?³Ó‡V?	¨?ï6ÿGÏ?–k0¬n~?™.@$ö>?–k0¬n~?ïÿÅm»wî>þ£3Oå	…>ýIB¼->þ£3Oå	…AGN3FGL J1643.6-0642@%"~e`­@8zE¿ý±qÀ9†ãOÆñÀ;…CÛ?™zVº@Ð@2*M±c»@'
 yó¿ìK1uT&.¿åw©Ò]'¿Ý|•DDº¿ÓÑýÀ¬ûCAGNbcu@±!¶E¡ÊÁPowerLawNVSS J164328-064619?ïù—Æ…µâ?Xï~w+±?I åÅùE?Xï~w+±?ïšêÈz?¡ðsÐDA?‰|C'¥)?¡ðsÐDA?`Îvñ?‹ö:ÖÖëþ?ŠØ§¾£ÓÕ?‹ö:ÖÖëþ?ïúŽ•ÉDF?3ƺ(?EŨ#P–?3ƺ(?ïñ¢€Y<î?i²Ârd¸?\ºÿtÃ?i²Ârd¸?ít¯P e?Á.>Û÷¦Ú?´Z…€´¥¢?Á.>Û÷¦Ú?îûĽ<i›?›ØÝ#ÛG? C´(ÉÊO?›ØÝ#ÛG?ïÓ6ø~p7?oÿ­ºÚÒ4?vdƒ¹è¬m?oÿ­ºÚÒ4AGN3FGL J1645.2-5747@t£½ßÉÿ"À¨
`+8éÀ9–u—5À;Í#3᯿ör25J@
ÝeÌ7§@f+ —ºœ¿é7¤
zœ¿êäT®-${¿à.­i"¿ç^瘙ÙAGNbcu@†ÿ»â.]áPowerLawAT20G J164513-575122?ïù—Í†A?QµÆÀ(,¥?I¡ø{I"?QµÆÀ(,¥?﮶hÔ¢&?"í†díò?"ReÑŽ?"í†díò?ïŠìW#à?…—´=êZ?Dê0Yñ?…—´=êZ?ïÿrå¶ä¿?Ô0‡Ž ?£C½úîy?Ô0‡Ž ?ïé¢+A)ô?jq'lâòu?f]Ô¬ø ?jq'lâòu?í>â¶Ãöå?Á3DMëMõ?¶êK˜Ó?Á3DMëMõ?î±G?|;?™oº3SOÄ?¤ëŒ	R?™oº3SOÄ?ïôÈqüÐ(?SFÇπ:?Vo¯?SFÇπ:AGN3FGL J1645.9-5420@tÏß֔ÍÀ'`óÀ9?‰i ­ŠÀ:æÂ:¢"=?î¨JG³3@Ȗœº
}@¸€nz\¿ÛŒ8óf"Š¿ìŠ!n«¿é3BL«ª=¿ïþNh†ÒOTHERspp@ƒ™™™™šPowerLaw?åf‰¤Ùê?ÉÈöÃM?Õ3Öì¶L-?ÉÈöÃM?ÕÂæ'Ää?ËGà>n¦?åö·Ž?ËGà>n¦?è»ó⡆‰?°ë¿Rd ?Í0uyåÛ?°ë¿Rd ?âG'*xh?­DÛJj¼Ÿ?ÛpÝÕ«/?­DÛJj¼Ÿ?Ø0-@L?ÌYO5·
Ý?ãçé_÷Ù¸?ÌYO5·
Ý?¥
]!ÕN?¶TûY¿?î¯Z.'cO?¶TûY¿?âªlN÷?¸	núk?Ú«õï'b?¸	núk?µ£Eõð—?žXþV¯$ ?íK—A
ó_?žXþV¯$ MIXED3FGL J1645.9+6336@W‹ž_Ñ÷¯@Bó©?ÿÊPÀ9ÑaE•5‡À<5ŽWF8¿íÍ2Ñhà@kC¡•f"@|/@_k ¿æö~b—µû¿éÆVv·Êæ¿æ_o¯:jµ¿ê'æ½õՖAGNfsrq@|Llß&k¥PowerLawTXS 1645+635?ïÿ¤Š…ÌÕ?ç	ì<?Ý^{3?ç	ì<?ïàAù8?€o¼{Èڙ?oá¾5'0X?€o¼{Èڙ?ïԂelã¥?nlÓ_ó?u¾ÍFÎ}G?nlÓ_ó?ïÿz/à²!?çÔN®xm?¹üP	ÉÝ?çÔN®xm?ïÿÔF=Ñó>öęIØ>>õÜÊá;Fx>öęIØ>?ï0є»A?¬"<¸´¬?™åÍh—ÝÇ?¬"<¸´¬?ïáâ¢c?qšKg?no"'…/?qšKg?ïøoµÄ?H:-Ì4­!?NC­Ñ'5ê?H:-Ì4­!AGN3FGL J1647.1-6438@tOÞ²gÇÀ(Þg@€ùÀ9»†ÜþsÀ;•BâL'ÀxwRœÚí@Þ
ô¸@ƒÄ`Á
¿Ü€Õ$V˜à¿å.ߥRƈ¿ã½Kõ÷¾h¿Ýÿ¦ù¬ÕAGNbcu@›­ß;dZPowerLawPMN J1647-6437?ïþ¼od^? §ûê–b?$>[TݾÚ? §ûê–b?ïÀt¶zÜ?Ž²ƒÇᅵ?ŤÇ™í?Ž²ƒÇᅵ?ïíHAڍL?]YI–Ш+?b·¾@?]YI–Ш+?ïÿÿÚô¶S>x"KÖ¨>r~Y¥îø)>x"KÖ¨?ïþǟwA?"q×X;?#†}q|?"q×X;?î'dÔÀâ?¼‰QÚµ?­ù®hnå?¼‰QÚµ?ïÊÈ<wÞ?~gF±¥_?zöÚäÙ?~gF±¥_?ïÿúdñ­h>ÏØ:&¡@¸>Ækkr	9>ÏØ:&¡@¸AGN3FGL J1647.4+4950@S)®_ú;›@DvŸ™ÛÀ8¢ßüTÀ;±m«Õ€?ëO§Á‹·?@<yX@nÈáÉ¿ä»ôbgÿ¿æüÓ¦8l¿æ"ÑËAæ¿äð滜‰õAGNbcu@²5\)PowerLawSBS 1646+499?ïÿc-Ýïñ?[9«œCJ?š@3 èä?[9«œCJ?ïƽ䧉ò?ˆû©Ó$_?|¡
´zÜ?ˆû©Ó$_?ïØz€èP?jÙIîò¢°?sÂò±ÍgÞ?jÙIîò¢°?ï'ä	ïö?kÅDBO/é?‹FýŽVR?kÅDBO/é?ïþXEVn?,"úó?*¼¥IoL?,"úó?î2à6áé?¸×Qev?¬Þ±ÿ%–f?¸×Qev?ïœR¤Z?….r'êd?ˆà+aH=ˆ?….r'êd?í7rUˆ×?££ÈÊô*k?¶DmRŸÒF?££ÈÊô*kAGN3FGL J1648.3-4611@u6òä¼®¿é©Ùà(ÀÀ7ü¼b~À9íý©
ªã?ý#íãr֌@½•6Þcx?õ:7>/»"?ïò¦æ‰6u¿ÁIYvz¿ÞSªL^¿í‹9Ëím›PSRPSR@§`6âëPLExpCutoffPSR J1648-4611?!½ž?7Ñÿ‹ ˜R?ïþï—'#…?7Ñÿ‹ ˜R?¬NR«í†?ÃæŸ=ò2?î;êð¾?ÃæŸ=ò2?³ËÏ$T˜ë?¤!ÇåÝ??톆Yð?¤!ÇåÝ??µdó;úÁ£?›*Î1ª1?íSa˜e*ì?›*Î1ª1?/'4c^À<?&u™»;?ïþì‹â?&u™»;?Š»C0­ý?§[¥¾Ò'?ï•ófƒ\?§[¥¾Ò'?¤–]ÁSÐ?£¥6Šõt³?/ãêÃ?£¥6Šõt³?'De"í(?€~í ·-?ïmÜÓfU0?€~í ·-PSR3FGL J1648.5-4829@u-••ÀxNß·
CÀ8»
Z[–)À:m‰;}…?ΨÃ:VO@	R|N°@N wm?écØÏ[꯿î,™¥qØÏ¿ÓXå~
eÞ¿ã%ö 'AGNbcu@–È—$tTPowerLawPMN J1648-4826?ï]Í_2¯D?šŒ§ö¿?"FTaå‹?šŒ§ö¿?ïfõ'3ö}?¢V©£à–ï?"![¨še?¢V©£à–ï?ëFÚZ‡"?¯j5tsGà?Â䖕᱿?¯j5tsGà?ïÚ¶æDð?XÕ`¶?r¤Œò®< ?XÕ`¶?íïì‡?²%ñÂí©P?°‡ˆŸ‰8G?²%ñÂí©P?ës>iœÚ?Çêy!Uo?Â3²YŒ—?Çêy!Uo?ê¼t¤äó­?°§p­?Å-ll1N?°§p­?ï^¦·[Ä?€³ÃƒþH?"<ë)‡ˆ?€³ÃƒþHAGN3FGL J1649.4+5238@T}òÿf@CÃÙ?¡ÖÀ9'm;l¾À;ÙuxR!5?ïdí·ËUK@@¸Í'n@À@Že‰¿Õiïk¿áp&ÛèÛ¿å©
O…
¿ç½LþµyAGNbll@"F§ï²PowerLaw87GB 164812.2+524023?ï÷Ï¬Û?R8Hb»?Pü`,HY÷?R8Hb»?ï'›3Þ»?'/™[íLÛ?
¬"\¾©?'/™[íLÛ?ïpi?ø?Š›5²ό?'ýòÌ 3?Š›5²ό?íãmì¨Æn?†¼¦'/Û?°ä™oò?†¼¦'/Û?ïňz¸Wö?€l$¨@O?};Œv­F?€l$¨@O?ë'÷é}~þ?¿]Öh	²9?Á¸ Z
?¿]Öh	²9?íW.j™Z?ªöêÆV?µFl«54?ªöêÆV?äl`¨®­?²6t}¢º?×'é>®¢¦?²6t}¢ºAGN3FGL J1650.2-5044@u.ŸðË°À«ÎÀAùõÀ7©ZÎyÀ:©6»}ïð?ÓÐӆi)ÿ@Ÿ,¾O¢@]'ßæÚë¿ä÷*JY¿æMc¡ÅÍ¿âÎÖ£vx¿ãZ/ðCۈAGNbcu@'‹ç»/ìWPowerLawPMN J1650-5044?ïü¸è"SŠ?>ˆ—s€?:8½{rÝ5?>ˆ—s€?fZi?'ؗ3Í]?‡f†¸9š?'ؗ3Í]?ï3~–?•K†¶Ÿ?™œP2fge?•K†¶Ÿ?ïý‡žß—? IßM»­Ñ?3ÃÿaJL? IßM»­Ñ?ïóiћ?c\ª:O«ë?Y-òZº?c\ª:O«ë?ìJd÷"[?ÆnUle{?½¬Û€CÝ%?ÆnUle{?î}íŽÝW?¡*'A3òŽ?¨!'u–?¡*'A3òŽ?ïö\•N¨§?H:ëúèU?SFÕº¤±œ?H:ëúèUAGN3FGL J1650.8+0830@:œò?Mé@>¢	Às"7À9lž#lÓÀ;nâO?ä~Oz!ëH@¢€Èè<@FÀ—ŠK¿åø~¡+H¿é§ÅËô<¿äIFɤ4Ž¿ïÿi¢¹†AGNfsrq@|ãöy|ÄPowerLawMG1 J165034+0824?ïøµ,‹èñ?KåÇá•?M+MWiýÙ?KåÇá•?ïfµñ$V?š+aµe?"=É@#§<?š+aµe?ï'XU_5£?€¥pŒ5?‹©êãÃC?€¥pŒ5?î£kd§õR?"^è½a'?¥ÉI²ìõä?"^è½a'?ï÷"
]žc?TúÿtC»˜?P÷ë!Ié?TúÿtC»˜?ëdÇ4²dA?ÃJÂòGä?Âlã-6ný?ÃJÂòGä?ïéIã¬k?–åh²Ãx?ŸÂÖÅB@¢?–åh²Ãx?çK"S'+ð?´¬"V»Wí?Ñh×XÛ¨!?´¬"V»WíAGN3FGL J1651.6+7219@Z³¿µ@AZ–`)5ƒÀ:ÌÄbšÿËÀ<$#wÔLô?Ö.u{N¢G@
êO²¥"?üÍ+4¾y¿ç5Œåj¿ÞR´úw뿳d™ûœÌˆ¿ÙÕ~5©É×AGNbll@µTG-PowerLawRX J1651.6+7218?ïþ>,ò?1½6tÊSœ?,20â?1½6tÊSœ?ïÖnµ{ˆž?'¯RpÄN?tÈ¥(©M?'¯RpÄN?ïÒòº-t?zÉâ?v†¢éõâ¦?zÉâ?ïëø¹˜?M¨pΉ?dïoÕÌÿ?M¨pΉ?ïî´d\\3?b ØA½í
?aK›µÅP?b ØA½í
?î»]º
?°)ª‰±
6?¤J#Öó?°)ª‰±
6?ï"AÎ2?Ž`~ŽÞý?Šï»ׁ?Ž`~ŽÞý?ï'-K+'B?'ÔöÕE€?‹´­']?‹?'ÔöÕE€AGN3FGL J1653.9+3945@OËôàM/@ClصýÀ6ÃðÈT˜À:(3Auì¿òBªפ—@ø|¨òþ?ûv'¿aª?¿×Ò9M¿ÜU,Ò,C¿ÒϰōÆÛ¿Ó%°)d8 AGNBLL@ 
ž5?|îPowerLawMkn 501?ïՐ‰`͆?ŽgàŽö}u?u7»?á?ŽgàŽö}u?ïÚÚoÞÆ[?"…·G©?r'È<ú­?"…·G©?îÇk'Úÿ.? {ýØVšv?£‰M"ãÂ? {ýØVšv?ïÿþ
">³ø-Ug>¯bTÍIÁR>³ø-Ug?ïçH,OÐ^?néozÙL?h·Ó¬ù?néozÙL?îȃ¶r1:?´½{êêÂ?£wę¸Óe?´½{êêÂ?ïLy*cV?"KxíøM?pØûÇF?"KxíøM?ïÿ÷öµî(>Öeþ°$¼>ÐjîµÚº>Öeþ°$¼AGN3FGL J1656.0+2044@DDãõhÍ@A"'@	‹À9¿å¯ò¡sÀ;±b'¬K¿Å·zº9ñ@üZNU"œ@ñaÿÏX˜¿ãi Æxd¿è%/u5)¿á¬@ÒFøý¿å '<9ÁAGNbcu@†ξߤ@PowerLawMG2 J165546+2043?ïÿéÖâ"#>édt% >æ)WßÆ°ì>édt% ?ïÌ¥Ze?'OÕì‹M?yô-W‡Áw?'OÕì‹M?ïíö8^žÏ?`d^–'¼?b	Ç_h°ï?`d^–'¼?ïüû4­öb?"ŒT1K1R?8&Yö^s*?"ŒT1K1R?ïÿãl˜Ñë>îò®¬ËÝ:>ì"lJðé½>îò®¬ËÝ:?î±àÂSà?µÁÊKmÒ?¤áóÆþÚü?µÁÊKmÒ?ïӇ0áI\?y6¡þF/M?v<gqÂ`?y6¡þF/M?ïèñ3g=?^bað*?g̞l"Ñ?^bað*AGN3FGL J1656.2-3303@uépÀ&Ì@`™?׆dÀ8Rys‡À:æ#wÔLô?sÒ­@³ožss@9·?œÎ¿çšç{¾¿éõÉß÷;¿ìŠ?£GÜý¿ïÿˆs¬uAGNfsrq@x5-PowerLawSwift J1656.3-3302?ïúŸÛt|Ì?c)e?E€'À¦
y?c)e?ïfXÒ)- ?£þϕ‰Q"?"4å³û$?£þϕ‰Q"?îN»œE=?š¸Ñ"1"?®»BÌ6?š¸Ñ"1"?ï\æ®RìÀ?uÜcÞy?"c*:ÉÒ?uÜcÞy?ïòôwÇÈè?pã³oä?Z†k¯ž?pã³oä?ë¡'Û¸?ÄqÖåïo?Á{›cÀ'"?ÄqÖåïo?í˜ÏaI?£ãC-gœe?³9"õIx?£ãC-gœe?ìd$²‹?©5&o®Î/?¿ÄÞßÒk¦?©5&o®Î/AGN3FGL J1656.8-2010?ñŒlà@,%8@¹-´À97
ðôÊBÀ;/[àÑf?ô²Ãú@Mx@òûûcŽ?ÿ`%ßãí?ïÿ›BÞnW¿Û9'lIF¿àÿ£¿é׫»¸°êAGNbcu@¤!WOß;PowerLaw1RXS J165655.0-201049?Õ½¼N${4?ϙd•€Û2?å!!ØíÂf?ϙd•€Û2?ًÃTEä?ÒäçW´ê$?ã:sÕÝ?ÒäçW´ê$?æ‡á{$'?µ¿z~Ì9?Òð=	·±?µ¿z~Ì9?ãç
¿\Ýã?®é?
çì?Ø1êFD;?®é?
çì?¸_ÜÐa=?¾•í³?ìôe¯ -?¾•í³?Í»Ù×Ě?ÐocW2?è 	ŠÚ?ÐocW2?̒¥|¯[«?½÷9ƒ•‡w?èÛV Ô)?½÷9ƒ•‡w?ѝ·*Ï–?±ÊPE½¤?ç1$j˜z5?±ÊPE½¤MIXED3FGL J1656.9+6008@VbøÌN"@Bµ²€l"À9Û²~líÀ<ÇC ¿Ð÷Q¼qq@'¹E†qõ@ûkŸ¶>@¿å eJT…¿è"²ÉF¿ç©ó_n᛿àßZYAGNfsrq@"3œ¿PowerLaw87GB 165604.4+601702?ïÿzd}¶˜?G	
#>$?³r¶."?G	
#>$?ïÚ#+Bâ?ƒ™wˆNä?rîjHI£?ƒ™wˆNä?ïçm©"Q?_"ÕtZ€?ho'e™÷?_"ÕtZ€?ïù$J¦Ü?6Ü«›Ö¬3?KnÔd`ú?6Ü«›Ö¬3?ïþãÀ"??%·VÓcâá?!Ãövš!«?%·VÓcâá?ïZŽÁÏC?®V	¯¨ºú?œt®"ž­®?®V	¯¨ºú?ï×r®¯fœ?v{Ì¥G"?tF¨¾R?v{Ì¥G"?î/·Â?'ŸBݜæ?ŒVDtf?'ŸBݜæAGN3FGL J1657.7+4807@R–»À5Ö@C>'ŸÐ€À8¥Þzt:dÀ;³r–'–?×Ü$÷ŽÊç@\z–9ý@ÍÖ©˜¿ä…ˆõ lÌ¿çEȊ"(¿æâ°ä0c¿âcóü«P•AGNfsrq@€ÁՁ%PowerLaw4C +48.41?ïÿÂÝ# Þ>þßÈM¸q>þ'O¾:xC>þßÈM¸q?ïÕsðËZ?‡Šwæâã?uFëk§N?‡Šwæâã?ïá²S
$W?eÆBí*e?nM¬¾áèî?eÆBí*e?ïýì8?äUå;»›?0Š<G«5@?äUå;»›?ïÿ|~8?I?•˜ÆGD?I?îÌÿ«­~?´#óàÛú?£0A¸{?´#óàÛú?ïÄZ"—Ò?}âûæRsW?}ÒñÐw‡7?}âûæRsW?ïõ'Uyüh?OÏ_¨?TÛTþHÀš?OÏ_¨AGN3FGL J1658.3+6149@VåT¿àU@@Bwìàh‹À:•€,
JÀ< œé°2b¿èl?Dþ%¤@¢A]îH@:»?†¨¦¿ê"Õ0.Ø¿ÜðÙ",¿ÛK€:;Õ¿Ö:µ-+AGNbll@¦ÕÛÀ6ãPowerLawNVSS J165808+615001?ïþE1by?3±šoå.Ó?.»©h¤á'?3±šoå.Ó?ïàjâ)³á?|Å& ì]?o•Ì­6ì?|Å& ì]?ïÚt´Ì"²?nY4™û—M?rÅ¥x¹f÷?nY4™û—M?ïþ/l€î?CÀ›gì?-E§XæÍ?CÀ›gì?ïó¶%<?[ÖÝqˆ¢?X"ËÃE6+?[ÖÝqˆ¢?ï-0|õt?¨3DÖµ?šYð]áâ¨?¨3DÖµ?ï®4ù±Ý2?…~áMz?"rÁ•ðmj?…~áMz?ïÞê¨n¸^?m=\òì;"?pŠ«Û1´Ä?m=\òì;"AGN3FGL J1658.4-5323@tíÏàGÓÔÀcð@uÀ8ž•Ï	½ïÀ:ðàŸèh4?þ-µÛC³@
¶tñ™‹?þó`Åg¨±¿à_Âáø"7¿á¥v»¿êù"iiü¿îÂi'¶ºMPSRPSR@ì˜~|âPLExpCutoffPSR J1658-5324?8{mB°&÷?M	 ¡û?ïüð'5…?M	 ¡û?¡ÔŸñJÑ"?¼ÜýË·é?îⶎ>?¼ÜýË·é?ÆÿX`› ?°22?ê@)ü'Ù8?°22?¡)©}¯†ª?'iC3[)?îíeh\U?'iC3[)?@B(7?A'Çåõ¤E?ïûï{½)…?A'Çåõ¤E?™Ë	±¸?«écöéc®?ü!	?«écöéc®?¨Ü[·Á	ç?Ÿ_—¦ªm?îr:DŸlA?Ÿ_—¦ªm?aÚ K?S†ÝãùÇ?ïî%ü$9?S†ÝãùÇPSR3FGL J1659.4+2631@Gŝ¿™£@A¢¼ßï¿@À:Lyãñ¬€À;¾†ß'±÷?×ýißäùâ@ΔY=ÞÞ@­–@ž«§¿çeXøŸ¿äKÛyý‹Ë¿é³_
|…¸¿ØÙ,¸V~AGNfsrq@@{çl‹DPowerLaw4C +26.51?ïýÚ¦ ²õ?4nI¢ï"—?1*ÍÛo]8?4nI¢ï"—?ï­x8jø?›ÕÓ-Os¥?"¡òSMã?›ÕÓ-Os¥?ï«1O5ûÃ?{"xc0¬f?…3¬$ŸP?{"xc0¬f?ïÏøT©¿E?blz®p6?x՝aí^?blz®p6?ïíS>O'?lÔö¡oÌ?b¬ÿÅÐË?lÔö¡oÌ?íÇðGâS?¼=c"d-ý?±Ç@x»f?¼=c"d-ý?îƒ.ÚÍ°;? TÒì?§ÍP'GN? TÒì?íœÐÐèeZ?§4Ö7û?³yx¼Õ3?§4Ö7ûAGN3FGL J1659.7-3132@vØ¿p@¾$çùÀ9;\WìÀ:úszK ?ØY¬Þ^´@
<În7–@7ˆàcØm¿ãV<=%­í¿éÙÿÒL'S¿Ôš©ùQÿÁ¿ëR@¶˜GAGNbcu@""Þi­BÄPowerLawNVSS J165949-313047?ïŠå'"½g?–®9ŠI?F›¡¯ÞB?–®9ŠI?ï=L2¢Xt?¤Ha0ìÔ?˜Vy©ý#‰?¤Ha0ìÔ?íX&*È;Õ?£4ßòΧ?µ>ښZ?£4ßòΧ?îìãQ¸HJ?"¶TO†#?¡1ÊèÆþW?"¶TO†#?ìËÒã?ºf'3)*Ï?¹¡hã÷¿G?ºf'3)*Ï?æ…ç!ÚÑ?ÍçØ- n—?Òô1¼KÜ^?ÍçØ- n—?鳺EûP³?±[Né`+?É1è½6?±[Né`+?èz‹òg/?¸zV;k©?ÎÐ6c¿B?¸zV;k©AGN3FGL J1700.1+6829@X⪀J@Aš¸GÀ7õKÏknÀ;2ƒ
?ñs¯g6@šÿ¬óéq@/EnÛ*¿ãúpø]¢¿åÓFœz'A¿æ`¢›æ¿ê2.™AGNfsrq@"FsØPowerLawTXS 1700+685?ïüM‡-—y?8c4§¥ŒÁ?="ÇJ≓?8c4§¥ŒÁ?ïÜü]CÆ?'Ê‹ÁÈ??qÑcÐØø?'Ê‹ÁÈ??ï'+^R›®?‡~7bÅa?‹µ(y"[?‡~7bÅa?ïþ]ÿm; ?ã{øØ?* Ïêž?ã{øØ?ïùäX=?OJB̳?Kàoƒ
'Ž?OJB̳?ïL;¿–$ç?¤e'=]M?–xˆó1?¤e'=]M?ï@ÿê†q?'ºbNð!<?—ðfÿÚ?'ºbNð!<?ïý#ÈՎ?55Tüš'÷?6áÀ7˜\?55Tüš'÷AGN3FGL J1701.2-3006@v{ 1ί@=ñÀL5äÀ8™'è|U¼À;§ú…l¼?üê·
ÈÀy@ÉþºÛˆ§?øDÓò0±¿Ô'\лnÖ¿àÕë/³L¿åÁáìï'¿éœ!3OTHERglc@"ɤxGLogParabolaM62?Å{½P-
?ÇxÎÊö*a?ê¡«ôºý?ÇxÎÊö*a?°'Ýš™V¥?À…½wLñ(?íï¤LÈR?À…½wLñ(?ÚFÐEʆï?¸®%¹­H>?âܗݼ‰?¸®%¹­H>?‹Yv$0?Ÿ¤Ç¦ñf¢?ë[Ý)¢vô?Ÿ¤Ç¦ñf¢?‰²ÁÁ}z?'Î˯µG?4ë;š?'Î˯µG?•eXS¼M?®% 0^-?ïTÕ=oÞF?®% 0^-?Á%ƒ[a?¹ýÔñMN?붹_)'¹?¹ýÔñMN?}ô(Œ?{.Âáv?ïl–È{?{.ÂávPSR3FGL J1702.6+3116@J³Ÿÿå(
@Aá.ßç[ÄÀ:T'Íó=zÀ;Øèd?ð¼48Á½z@Ó/ Tk?öV‡¡ž&¿ëRHíã%‡?ïøvP`·ó?¿ØSË{‹^?·%ÂåËÔÞAGNbll@®vÈ´9PowerLawRX J1702.6+3115?ïª"ɽÊ?J:ûmc?…wM»àñf?J:ûmc?ï˜"på"?›Õ¸ÏVú??‰þ÷q…??›Õ¸ÏVú??îÅB_¦ü?˜êQdn?£«ßL™E=?˜êQdn?ï²ë[XŽ?qøË"f¨õ?ƒE:u0~"?qøË"f¨õ?ï¥5(MH€?ŒðõîP¢?†²µâ_(?ŒðõîP¢?íXìŠy¸u?ÀÈùûi?µ8›ªznY?ÀÈùûi?î*0]Ég?¡>aéÃÂQ?®=\ý""?¡>aéÃÂQ?ïb¤š©?%‹Üð]?"«l®=»X?%‹Üð]AGN3FGL J1703.6-6211@t'%¶™…À(Ü>úç'À7ðª4À;?úVôÙ?ìÔ:>a±î@…g;Mˆõ@È£Ìhú¿åE:‡:qk¿æU/ø¾¿å²Ê]ZÚ¿ìÒºû15AGNfsrq@€
º>À/0PowerLawMRC 1659-621?ïã%ˆòú«?h6ói<,?lÚvéIdã?h6ói<,?ïœgÀè? Ñ¥ä%ú?ˆÿæ<–? Ñ¥ä%ú?îƒÊœ"?™Œå'Ûyÿ?§Ã_|šÚ?™Œå'Ûyÿ?ï÷^üd¿ó?:^´•Ï	›?QB©òù!?:^´•Ï	›?ïÐ!¯¨$?x?ë	ô)™?wôo'|?x?ë	ô)™?íq'vE½¶?À¶ ªHØ%?´stLˆ7Õ?À¶ ªHØ%?íÜ0f
‡)?¡T/Þä?±|Íóø½?¡T/Þä?ïç‡Á9,?_z`»£üì?hxìV$+Þ?_z`»£üìAGN3FGL J1704.0+7646@[;ɟâÚ@@3S 8"¬À:gCÛ÷ãÀ<´SYCh¿ÙúhöRq@"cW=@—$ žE¦¿æedÿð ö¿çaÕN•S(¿æõ47?1n¿ïþëWýBAGNbcu@'Zü@ŽÉPowerLawNVSS J170357+764611?ïÿ®÷NÖ}?•_ó¯?"?B)Š°Ð?•_ó¯?"?ïÝ«þ7?ƒªÃ<ʏ?q*~æ³Pk?ƒªÃ<ʏ?ï·éIôÚw?x{ºE÷x?'­"P?x{ºE÷x?ïý È?§é?)Ud&Ï?2ù¿Í?ƅ?)Ud&Ï?ïÿÚeÌ>ôÑx£×>òøå,^r+>ôÑx£×?ï‰Øí}®?¯Þc/Gø?nÄÛqW?¯Þc/Gø?ïÏK-êÂ?}7Þ9ðà?xZhðœH?}7Þ9ðà?ïäܮʶÑ?bV&4d?k#Q$Ë'?bV&4dAGN3FGL J1705.5+7134@Y¿B¿˜0ä@@õ®Ú«³À:¶ïº€À< VrÓ\3¿÷ýò ï8Ý@ùÛQÊÍï@'¿_Ñ̼¿ç[¸b‡‰¢¿éeÈ­´¿¶x,rµæ=¿ïÿ"m¾RAGNbll@džDúPowerLawGB6 J1704+7138?ïóY¥U?|'Ü_ížz?YL¶J€?|'Ü_ížz?ïÞ46φ!?'X7Òú£?påä€ß—·?'X7Òú£?îÄ+ú•ï?£*äT0?®ó½=Âì?£*äT0?ïÿ0t‡Û?6&4¶?ñL0j?6&4¶?ïޞ*än?ƒ³€œÈÐ?p°ê߀…V?ƒ³€œÈÐ?ïMˆ"†y?Ÿ×H)N'â?–Nïxߔï?Ÿ×H)N'â?í(¡¡û½Ñ?¯1Ì551‰?¶ºòïF*y?¯1Ì551‰?ïï‹þrى?cþ÷@º—'?`t"çgL?cþ÷@º—'AGN3FGL J1709.6+4318@QŸÞW9@BƒÀ€æÀ7ÇÎÄô'7À;7[‹AB?ö(ƒFÆãÕ@b!LÖÈ@Z"tf"¿àóÛõ3É0¿ä³"›Çµû¿äÛÖS‰?¿éU*m¬AGNfsrq@x©,ÄLogParabolaB3 1708+433?ïúHø[4É?GH8 ?FÜÌY«?GH8 ?ïÏ8‰Õ=?‡›U½i?xcòÚ݉?‡›U½i?ï¯h]¸Ý?€îë¬Ëu?"%ù³8'Ë?€îë¬Ëu?ïÿš^)oÕ>ú—©'Úv?	hu‹¨R>ú—©'Úv?ïóû=+7D?Xzô†ÝÑÃ?X	†	Ƈ¡?Xzô†ÝÑÃ?îñÂðªøg?«ðyšÄ? ãÐ÷ä.'?«ðyšÄ?îöSŸËs?˜ˆ ›7Í? šÆ¸j?˜ˆ ›7Í?ïÿ©Î›&?¹mwì?Œ]ÿ¶`À?¹mwìAGN3FGL J1709.7-4429@uq"_ôöÀƒu€_¶ÊÀ4s 	ŠÃ=À9Œ";±†ö@
Êϓ%·@îô¿ÚöÜ?ô…¼/E½Ï¿Ñ3JøLt¿ß[o˜ÐW,¿äDb"4o¿ëž©<·ÁPSRPSR@ŠŠN_oÒPLSuperExpCutoffPSR J1709-4429?3G€›Ð?8ï÷HÒÆ?ïý—ÚH?8ï÷HÒÆ?¥-h«Ö-?ÁOŸ¹Í?î­)u^Í?ÁOŸ¹Í? hH­‡¦í?œ4;rè?îù{u'…'?œ4;rè?ÿ[ãT²ˆ?"a)&k?ïÿ@9áß?"a)&k?<ú'Ñ¢P‡?En¾ÊÏ?ïü`ºÄ¦Q?En¾ÊÏ?Ž	Ý_¨Be?­°|D€)ß?ï‡ØŠ^ö?­°|D€)ß?yõe{ò?zÚu"p&¼?ïÌÛð'`?zÚu"p&¼>î5N7èç>óÜân¦¤V?ïÿáÊ_à>óÜân¦¤VPSR3FGL J1711.5-5029@u&¸!ïÀã
é`À9W4Ïëe>À:ûy€žQ¿ì~Ì¿%@÷þ;¯®"@võ_"
Ž¿å2­[O¿¿í"š¿\æ¿å$˜ÎmG¿¾•`åHÈAGNbcu@Œ²Áü2PowerLawPMN J1711-5028?ïù«!×@C?Iç2¨/C?ISxÞëUð?Iç2¨/C?ï¬kœ
ð·?'÷æ'¨Ð?"åò4þI?'÷æ'¨Ð?ïAÈbëî·?' mÁvä?—Æ󧩓?' mÁvä?ïÿÑ-Ñì¿>ìtHwAf>÷i
ó)Î>ìtHwAf?ïé4áÖk©?gø]þ	%?fË*ô.•?gø]þ	%?ìÑ6
®y?Ãü'Ì"¶?¹vO"G24?Ãü'Ì"¶?팇ïr&?§ªÜ
ç²?³›À‰â0P?§ªÜ
ç²?ïý
¬?5,Ðè˜3Ù?7—{mü"?5,Ðè˜3ÙAGN3FGL J1711.6+8846@^kYáó¥@;£Ó £ävÀ:p*ÜLœ'À;Ï(†1?âSb;+ª@
>àI+m?ù€@'&5¿î
rÓ©'?ÚtDìÍ¿ªmvûßßÏ¿ÇöÀÍK^	AGNbcu@ÁAÂMÒñªPowerLaw1RXS J171643.8+884414?ïþ'È­êp?&&/×) ?'Ówî:´>?&&/×) ?ïÒÅɒ•?†}^üçQ?vsÕ¹?†}^üçQ?ïÜá'ïç?jÝj/øt?q>…L‰´?jÝj/øt?ïÙƦÂq?XÝðoÃú?s¬ÛÄ?XÝðoÃú?ïø }ìóf?Lí4XXN?M~	&s.¢?Lí4XXN?î½>£Ã'æ?±8ÄÁH[Ð?¤,ÅŸŸ?±8ÄÁH[Ð?ï·æý‹Â¨?ô@®֟?'@¡†Ô?ô@®֟?ïi<ÛÞ@?‡ˆwL+–v?'Ømý¥?‡ˆwL+–vAGN3FGL J1712.6+2932@Iýöÿ¦=í@@ ƒ?»òÀ:D,_Ú[+À;›Ýj©Â?èàðÑlwU@Öa¤J"?ù4ŸWž¢?Õ-­zË?ï÷NÈKD¿ä¯ÀU"ÏÁ?Écu‡ãÛÿAGNbll@»»v‡+PowerLawRX J1712.8+2931?ï÷ë°¬t?bµÜ¿g?P(Ÿ#âf?bµÜ¿g?ï²ýÁ-Õ?—SâmWx5?ƒ|@›»,È?—SâmWx5?ïa²³#¶ò?‹–oύõ¶?"É© °‹º?‹–oύõ¶?ï°1þw6:?uvuæ«­?ƒó€dš+‹?uvuæ«­?ï¹|×};%?">ôGë? Ê©T¬?">ôGë?ícª
™Ð»?Ácíê÷?´â¯«Ÿm©?Ácíê÷?îAÚ«n®?¡Ø{u¤ïO?«â_'G?¡Ø{u¤ïO?ílFiÄâ?³—­<Ãè"?´ÏCåp?³—­<Ãè"AGN3FGL J1713.5-3945e@uµ`ûH
¿ÞCë c¼'À7m÷¤ç«À9ڟ¹nK7?å…ø¼X¥!@
t×½ìŠ,?ùú¿˜†Ê?Ñ$†<oœñ¿åÅoá9k\¿ÐJ)"]È2¿¿þE?Ð$›OTHERSNR@Ë«=p£×
PowerLawRX J1713.7-3946?ä
Ph£,•?Ч‰P%Ò?×ë_.¹¦Õ?Ч‰P%Ò?ï/«á'#?´Ñf ±«}?žú
……‰™?´Ñf ±«}?ãŸûÜÀñÞ?µE6IuçN?ØÀF~C?µE6IuçN?ïR£æς?v‹+tÿW£?Œ«Võ€?v‹+tÿW£?á€Ýæ/0?ÎWVúžÓQ?ÜþEô3¡¡?ÎWVúžÓQ?èüÎM37?Ê÷pÀÐI?ÌÆË3£#?Ê÷pÀÐI?é?Ðz?³oOO:Ô&?Ë÷ó¾û?³oOO:Ô&?íÎÎ ? _]½Q?±‰Å·-? _]½QAGN3FGL J1714.0+0748@<È%ŸÌ¹'@9/(Ÿ[zzÀ9cÇÚõ"|À;hèz0H?ùÐÄÔú@
ÕÑò¦{)?ûڀ׫Íú¿äþ̍¦‹¿ÖêDEÃóN¿àfr†ýr¿îÂÖF¯MPSRPSR@•aïìVÕÐPLExpCutoffPSR J1713+0747?Ž
äp¾•8?p)nõg\?ï‡Ôn=«?p)nõg\?Âíî •²ë?Ë'µ/)í?ëD"wړE?Ë'µ/)í?Ôñ˜iÿß/?µR¢Ï,¶?å‡3Ëh?µR¢Ï,¶?Î"8ws\¢?«ã
¾ÚL»?èwqâ#(Ø?«ã
¾ÚL»?m©ë*Ҁ?l¢»¥¶Ê?ïâVšÒæ?l¢»¥¶Ê?­ô£Ó
?Âô¿~Ÿ\?î ¾EÂÏ??Âô¿~Ÿ\?¸=|5¦B.?©Âò€Öù"?ìøPy=û?©Âò€Öù"?¡÷@fâ?‹¥:¹CÀæ?îàŽŒ0‹Ÿ?‹¥:¹CÀæPSR3FGL J1714.1-2029@	µŸ´Á@%,ê¿üÚ²À9åRÒ4ëšÀ;;h7÷¾?ÙÅ¿'6{'@{6¢0—?õ€ïÿÕÙ¿ïÿñã?ïøËùo˜?Ù8'2"t?¯ÄõµE¾óAGNbcu@ÑÿÐå`A‰PowerLaw1RXS J171405.2-202747?ï÷%xµsj?`À!À/Š¦?Qµ¸Õ?`À!À/Š¦?ïPtÊWQ¡?±Ëµ`Ø/?•ñf¬~Åû?±Ëµ`Ø/?ïeB­'7?–¥õÁaD?sWªO¹?–¥õÁaD?ïü w•?.ÄH~ê¹??Oqãã5å?.ÄH~ê¹?ïìw|Z»Û?dۚŸ°?cˆƒ£äMS?dۚŸ°?ì•í6Çà?ÆóµuSzb?»P–Iǹ?ÆóµuSzb?ïab‹eyW?r4JÁa?"Ó®–Àq+?r4JÁa?ïú§rdc?D©k,ùz?Eb6ÃßJe?D©k,ùzAGN3FGL J1714.5-3832@uÆìà2Û?³´à
ŸÀ6‡à3±ÞÀ9©Þß)?úžÉ|5Z«@ìNµo¸õ@g(ñ:ë8¿Þ]›ç|¦¿â¥¯¢šÜ¿ã¾¬B鉜¿íÕÇGQÎOTHERsnr@'gö"FtLogParabolaCTB 37A?¤8çšVÏ?°ÏòƒÍ?î¼~Á¯•ã?°ÏòƒÍ?·vFê[d;?Áˆ»MÑøŽ?í7"´"y?Áˆ»MÑøŽ?'¼*àv?°šuzñF?éyPÐõGã?°šuzñF?ÑP";º?¬6eñæ%¨?çW¶b}"À?¬6eñæ%¨?a¢[™Š©\?aÆLÛÈä›?ïî]¤(œ_?aÆLÛÈä›?™:»¶Ñ˜!?¯Â§µà"õ?ï6*"W1¯?¯Â§µà"õ?±~±û
+?¨=£|\L?íÐ)Àë?¨=£|\L?¬óÒà?›'N‡2Ë?î0ÂѲuð?›'N‡2ËPSR3FGL J1715.7+6837@Xә`#VF@@äå@a À9˜hô¶âÀ;Û k°R?õeڍ)ɨ@üÓТ?ý­ËOt1€?ÃØÑgç¿åý–Pía¿å(z‹LÇ¿ã
¯ÃžóAGNfsrq@ŽûŸŠ	ÞLogParabolaS4 1716+68?ïþ±¡Ö²‡?%äJÀ¥ˆê?$åߢµ—?%äJÀ¥ˆê?﵀{¡/?‰©¼7ºh?'Ÿáž??‰©¼7ºh?îïUMdaÔ?"\ª>Ç)ä?¡
«*•É¹?"\ª>Ç)ä?ïå>náÆ?yËÀîª:¤?ŸãX3ە6?yËÀîª:¤?ïþÍàj…Ò?.ï
ØÙýŸ?#!ü<´ÿ$?.ï
ØÙýŸ?í×`É_4?¹tã¾T.Ã?±Dù¶
8e?¹tã¾T.Ã?îœ' Jñ?œ''þ
U›?¦>Öß³õ?œ''þ
U›?ë"l‰ž­]?©‰zg~?Á®MمJ‹?©‰zg~AGN3FGL J1716.6-2812@vRÿÚ@S@ä%_µóÀ8ÃÆé]ýÀ:Íõ`iÍ#?ñMD¼rŒ@ÜJ)ÄÊu@ê@¿Ê¿â¬
µe§û¿è&Õ¢}þ¿ãÕíݾŒ˜¿ïÿò"²¢OTHERglc@‰H"t¼jPowerLawNGC 6316?ëDP‰QÅ?Ç]"'6G1?ÁŠî½Ú¸ë?Ç]"'6G1?∆úäñ?ÉY´'º@>?Úîò
7Ö?ÉY´'º@>?éBUˆ{AÈ?­Í+âÿÏ?Êö©Þøß?­Í+âÿÏ?æ	$R+G?§ÿ!
2t?Óí·[©ýs?§ÿ!
2t?èå¬A¼ä?ϏP©T'?ÏÐiNùq?ϏP©T'?ÂSÄðÕ?Æ­âY"‰E?ëx+Ãߋ?Æ­âY"‰E?Þ"±3zg?¼ã•ïž'"?àô¶'fBÌ?¼ã•ïž'"?ÉNzRg½?­EÀ™¢N?é¬akf¼?­EÀ™¢NMIXED3FGL J1716.7-8112@s{ fèÀ7U* ½zIÀ:—íùm?À;Îú2`¥\À
ü¶!9¶…@
æÞÿ)k^@zñ –¸ê¿êÐ熿î'ß«¡¯?ès›s
"¼¿ç"!šYïAGNbcu@ªœ(r° ÅPowerLaw1RXS J171712.6-811501?ïþ`‡n½?)bg.ñb?)÷Š£ËŽ?)bg.ñb?ïÎB«Ì!?‡ü·ç†Ž.?xñÞ½W¿P?‡ü·ç†Ž.?ïå7â;ì7?ewô…Yåß?jÈŽyá‰?ewô…Yåß?ïÿÿýÚ>ƒ>4ß2¶€Þ>/!"«¬>4ß2µÈfm?ïþƒ»áÂþ?40«Œyq×?'Ä@üê_Ñ?40«Œyq×?îë1mÐù?³*µ
Ò÷??¡Lé l;z?³*µ
Ò÷??ïܦLc
Ÿ?t'׏	O	?q¬Ùâfìc?t'׏	O	?ïÿÿés_>x&mJsÜ>fªÊ)Ä©f>x&mJsÜAGN3FGL J1717.4-5157@u»`(^ÄÀ (g "I×À8›.­'tâÀ:îs#ä
×?íŸÃ'™þ¢@Í? §?@óNi¿áµh†•ö¿æqÃóà7¿æ6ö°RÄ¿ï1æáPãAGNfsrq@Pâ]yÑPowerLawPMN J1717-5155?ïÜ7Þ`Š?owÏÜUÃ?qäáÓ²Ù?owÏÜUÃ?ï‡DÈ1³?™l©)79†?Ž.Í÷-ï3?™l©)79†?îTԄba?š9ìÉÃh?ª¾Â¼\ê?š9ìÉÃh?ïøn'›°?6ý¸¤Ê?NDôÑLÊ?6ý¸¤Ê?ïÃþRçêœ?~¾qÐ?~֑Š%?~¾qÐ?ì«Í~"šµ?Äf3‰™?º¡"ë*[?Äf3‰™?í~…ëM&¶?¤¥†ñM?´Цr±S?¤¥†ñM?ïì4«¥­?Z§8ÌKß?cËT"U?Z§8ÌKßAGN3FGL J1717.6-5802@tÊ*Ÿ{ZêÀ'¦þÜêQÀ9KHÓ®hÀ;_	Ÿ»òŠ?u 5Ø
¥@÷¥LUC(@]€†£¿ä."Š]‰¿ä <Ð.Åտ䅄 |üo¿ïü¸#Œ:ûPSRpsr@ŠžLáłVPowerLawPSR J1717-5800@?íÝ*$Ž!?ÂïqÌdáÆ?±®m›w?ÂïqÌdáÆ?ï¢Ò›ÿáˆ?"•ˆç†??‡KYê?"•ˆç†??ì¡A°?¥Ú`xڕ	?º÷%÷ò{™?¥Ú`xڕ	?ïhTK±?w­ÌdC·À?'õn[Ç3Ø?w­ÌdC·À?èIt';¥•?Èo\Ä?ÎÚ/ci¬?Èo\Ä?ìÕ¹ãï‡?¿ìÎõÆì
?¿!R0àƒÊ?¿ìÎõÆì
?ç¤l5Þ3R?´˜2×¼Áœ?з'"C™]?´˜2×¼Áœ?édéëÿÌ?²Ò§ù2û8?ÊlñXPÒ?²Ò§ù2û8AGN3FGL J1717.8-3342@v/€Uûµ@ވj1À7,ò³"À:(zúr!†?ðäH™w@ðU+%É@HkÀmmí¿å—Ì<%—Œ¿é3‹fŒ¿å¢`°ì¿ê½]¡¤^AGNbll@ˆ‡š!ê5"PowerLawTXS 1714-336?ê*Ç&Î( ?Ë)—÷,6?ÇTãdÇ]€?Ë)—÷,6?ï$²ß2L?œóY=-ê?iªøîg?œóY=-ê?åÃ&ñ¹ô¶?¶(+¨†cµ?Ôy²Œ"?¶(+¨†cµ?ïäýé'î?Q'JÓÒ?kÑ ?Q'JÓÒ?î£J!X·Ÿ?ªµwã¿Â?¥Ë]ì,T?ªµwã¿Â?ì øgS™?ÄäyYæ®Ô?ºø;"Åc;?ÄäyYæ®Ô?è¹?ñÔæn?³m¹/bÎi?Í8¬fG?³m¹/bÎi?ﲖT.š6?sëü$?ƒZjï‰þƒ?sëü$AGN3FGL J1718.0-3726@u۔€u?IJ¦ ÷­‡À7¾"Xð\À:I窞¥?Æá-;¼@
Òfhe@+äU¿çß'¶ÿ¿ãáäŒ3 ¿ß"ÂÇæ¿âœúÂSw OTHERsnr@ªŠ\¬1'PowerLawSNR G349.7+00.2?é‹wª	Ã?È97?ma?ÉÒ#WØô?È97?ma?ïD\¸E_?¯n§{Ð?—~th÷T$?¯n§{Ð?äN•Aù¨?·ƒ¤eª±?×ÁbÕ|°?·ƒ¤eª±?ï–Qà"Í$?w	FÖ2?Šk‡ÚÌ· ?w	FÖ2?æö$‡±²?ÉeV€4W?Ò·þðœœ?ÉeV€4W?éh"ÿVû?ÈHÓ6&
^?Ê]¬§Ð?ÈHÓ6&
^?è1Sâ«0p?µŒّã?Ï:°uS>A?µŒّã?ì<T2öç?¦h 'û'š?¿æ^hHÇ?¦h 'û'šAGN3FGL J1718.1-3056@v0÷Ÿ©~@ !€ƒHÀ8É&رÝ]À:»_"K|?ä™fîC@ÂN™–@þŸßXë¿Ûi;9ßA;¿ëV¹"uÝ¿å#m\=²¿áTn‰ËpVAGNbcu@"2I…ðoiPowerLawPMN J1718-3056?ïî±Yåà«?e4'IB8?aN¥÷Ã<ø?e4'IB8?îÿUñ#CQ?±÷«¥°R? 
 ê\.ô?±÷«¥°R?íÐÞé>? þHC0nl?±y¶z(z? þHC0nl?îõ^¾Š¦?Š,&?(? ª§¹¦?Š,&?(?îUÿ—?­—·Ú0êW?ª¦ S›‡?­—·Ú0êW?äŔ$Ëͅ?Ð%‡!µ»?Öt׶hd÷?Ð%‡!µ»?ç¹T?ÐØÿ?¶ÊèCÿ;è?ЍW€^N?¶ÊèCÿ;è?ç®Gë?î?´ùج¾ŠK?Ñâ£p)€#?´ùج¾ŠKAGN3FGL J1718.1-3825@uÏÀ7"¿Ûe}`††À78CæߝŠÀ9¿6n@O@!w¤QX@î!è2-û?ÿ£NÏ?æl>;ÇMÔ¿âKW€–¿æ»\s¸"`¿ïIV^0ÎPSRPSR@"'ä%®æPLExpCutoffPSR J1718-3825?d€õ54?pWÞ
ºÁ?ïë
Þ;›?pWÞ
ºÁ?§jŒÊU¤?ÀÂìèåËæ?î‰W31t†?ÀÂìèåËæ?¦ºÌo.áë?  ÆSsàñ?î"S9
á?  ÆSsàñ?²pv–9†Â?™&Š|?í±ñ-"Ø?™&Š|?Y/±–4
:?f^Ìxšð?ïóh'0Æq?f^Ìxšð?Ž‰"äÛÖ8?¬>ÒFX?ï…Ù죊g?¬>ÒFX?Mö½gþ7?¦Ž¹Žþ÷G?ïJž?¦Ž¹Žþ÷G?'h¦	-I?…n,åXI?ïtºÏ@¼Ö?…n,åXIPSR3FGL J1719.2+1744@CÂIàâi@<A_EàµÀ8Ãp@Ú»£À;L':ƒŽ¿è*"öØ[@³>\;-@WhÿóÀ­¿à;Ý
·£›¿à%–¯Yl¿àÿ[Ikž¿ÛÆ;IheAGNbll@™8ÛšuPowerLawPKS 1717+177?ïÿ®gm2Å?٘}Ðf?f#uÄäq?٘}Ðf?ï¾'´`*ž?•w²÷¶ß?€vÜF¬~?•w²÷¶ß?ïà£FŸ)Y?r2ó"D"?o\¹¤.þ…?r2ó"D"?ïÿÿ^fà>‰}'Êžv^>".ª/':)>‰}'Êžv^?ïÿƒ÷N‰.?Ê¿ôÂ?*ƒ˜—!?Ê¿ôÂ?î"h›H?¹CbDŸ•}?¦É~'ç?¹CbDŸ•}?ïÛí´ÁW?u=~?r	t5mˆa?u=~?ïÿýüššË>³qÉH¦	ç>°ö³Î΀>³qÉH¦	çAGN3FGL J1719.3+1206@@ÜLŸëÃ2@9Ö4 ˜ü¼À9ð5³@3ÍÀ;~#yÌ?ÞüRF…@Q8!.£×@ŸŸ÷ג¿×r¯'¨ï¿åêà`ÓT{¿ÑŸ!='\¹¿Ø]0Ú_ÔÉAGNbcu@©ÃÀ[À7PowerLaw1RXS J171921.2+120711?ïûîT"3?JçìÄì?@GŸ‹Í&¨?JçìÄì?ïo¿-Ûc? ˆ7q­?'FKj—? ˆ7q­?ï·âéTþñ?‡¤`‡S@?'Ež	µÊ?‡¤`‡S@?ÌÀÎ?t®`5¬ØŽ?ŽLÉT‰?t®`5¬ØŽ?ïêÚN¤?m‹*ÿÔªE?e%ïw¢pÿ?m‹*ÿÔªE?ëu'Ò>?Ɠaw¥d9?Â)ô·Ͼ?Ɠaw¥d9?ï9þ¢÷€?'"â^s?˜À+ŸX.ò?'"â^s?ìÏ<û‡?ªÝöÒÆ9?¹†VkùL?ªÝöÒÆ9AGN3FGL J1722.7+6104@VŠÆŸ÷¬@AàP7PÀ9ó¡gÄ4xÀ;ŸáÝÖ
?ߑ±ÿÓ«@{7*ŽŸ@øýŸÓo~¿è‹t­¸¿êTÓSFŽ¿ë¤3Š\]¿ïþ™øRü@AGNfsrq@}'4ÂPowerLawGB6 J1722+6105?ïú›8ŸÈ?@¡R¢Ð[ù?E" ˜P?@¡R¢Ð[ù?ïº×VépÇ?‡PðÔ,?J*UÉø?‡PðÔ,?ï™$¨‰?yûSòLa?‰»6ÎþhA?yûSòLa?îÛûÉ2?Ý÷0gj·?¢@CqVÊá?Ý÷0gj·?ïôäü:ñ?WTȽ÷,?WÜ66DÍ÷?WTȽ÷,?ìxj%ýYv?¾Ìé…È´î?¼<®Ð4M?¾Ìé…È´î?ïD$IáJˆ?™ÔS´?—{v»?©?™ÔS´?å£8ú›?´×".ɯ?Õð¹Žà
Ë?´×".ɯAGN3FGL J1722.7+1014@@m ‹]@8M@LzÀ8ˆéR>'5À;86%UúÞ¿æä¨Y·¶@˗I]A$@`Ÿ l1,¿ßýZ¸w+¿çÃÂÔj>Ò¿àqaûƒÕž¿áÓðÇË'©AGNfsrq@S;çl‹DPowerLawTXS 1720+102?ïÿ¹M$>þóõ@$_'?¬Ã+c-\>þóõ@$_'?ï´ÿ/d`l?"Àe(•;?'À4/~ë?"Àe(•;?ïà{K-ƒy?qKm¹ÜM%?o"´».¦?qKm¹ÜM%?ïÿÐø«wè>çñ?sï–>÷ƒ =X™>çñ?sï–?ïÿ‰ì)é?	tpôå?
"îÒ5€?	tpôå?îq¢ò*KÐ?·­a]Ï?¨åÐàÊÞö?·­a]Ï?ïº%,µš?'Öd¬L+¬?v´îõ"?'Öd¬L+¬?ïþ§}‡ë?$,̦è?%ˆ+Á҃R?$,̦èAGN3FGL J1722.9-4529@uz!@W%À«"ÿٔ†À9ÍSÛIÀ:°;C¢ìÿ?ԋŽ®Ùò¥@
­ñœÆ@ÁeÖt¿ã@4}áb¿éÏ"¢¿³¿ÙwÜÛb½¿ïÿîbHÊtOTHERspp@"ÐÑÎ_PowerLaw?çKG§˜?Ў‰Nâ€?ÑÇip±îÐ?Ў‰Nâ€?îòj֍•Õ?ª0¡9Ë? ÙR"·±?ª0¡9Ë?縘ÎÔ ?´y%Ñe?ЎÎbV¿Þ?´y%Ñe?îÐñ@ãü?ˆ°–É >?¢ðëüB$K?ˆ°–É >?ægøHï?Ïú°#¸…²?Òý0oè#?Ïú°#¸…²?äJÕŸP?ÍÝèÇí¹?×kÚUîÁa?ÍÝèÇí¹?æ÷6Å[`Æ?µvZG-ÂÚ?Ò'uI>t?µvZG-ÂÚ?ççƒh;?ºß$'ҁî?Ð0ù/‰ãø?ºß$'ҁîAGN3FGL J1723.5-5609@të¿çáüÀ&IFÿ˜ÑóÀ9ç**¾ðÀ;VB7²ô´?°_홃Ç@Lêik@ñ ÀTnl¿èæ¯æfÿ¿êò­Ï†}¿Î}$ƒmj¿ç×a"¯­WAGNbcu@‡¦‡â'@¸PowerLawPMN J1723-5614?ïþ¬b–o?&DwUöÀ?%9Ùª"R?&DwUöÀ?ï¢,8©P?'@QûÇ?‡tñÕ«ÿ´?'@QûÇ?ïѳv?sY‰)¦?w&DßlZq?sY‰)¦?ïí݋‹äÐ?J%ƒZï¬?b"t°"Oˆ?J%ƒZï¬?ïýãÿ»?8»!€ÝÉ?0àcj&E?8»!€ÝÉ?ìnû&b¦z?™¾ËŠàø?¼ˆ&ÌêÌ4?™¾ËŠàø?ï8ֈWÂ?•iÄ-±?˜å.ì9Ç?•iÄ-±?ïP_"äN?\Eö6W?‹ëè%UÀu?\Eö6WAGN3FGL J1723.7-7713@s»	 'RTÀ5˒€ ¤PÀ8ê̵O؅À;nÐ6䘛?í¢ز¼´@O·3ÞSÞ@ü?¶Ï5¿åQ¶†íοâù)Î'¿éØ8Уhr¿êú¹…$öAGNbcu@…ÌÞ FÇePowerLawPKS 1716-771?ï¼~¸+?"+ÊeÁ´A?€àyZ:…K?"+ÊeÁ´A?ï°c\h-2?E¹=?ƒç(笁f?E¹=?îP῀½?œ'A­,E?ªÿÁã,
9?œ'A­,E?O!%j?f~6ìm'~?ˆl&ˆ™±?f~6ìm'~?ïR¹È?˜Š[¡"?•¼ˆÜÝæû?˜Š[¡"?텔ý±#×?ºÓ=s±±?³ÓXšúE?ºÓ=s±±?ìYûÁNa?©'nö&<?¿U0!õŒù?©'nö&<?íÑv.tK?šHpdʍ‹?±w"OhD£?šHpdʍ‹AGN3FGL J1723.9+4004@P8Z€¶–@@–ôÿñ½GÀ8ÕÁw.4ÇÀ;¨"Æ£½à?ó0ºø¹å"@¥³ŸTD@œÏÀr "¿äs°¢"¿å›{4îc¿çÂá_'
¿ïÿÇ/ß_AGNfsrq@'Mj~ùÛ#PowerLawS4 1722+40?ïúŽu	}"?cNkôËé€?EÆ+F'P?cNkôËé€?ïÈh‰¬;³?‹/ÚºÖh?{Ë»J.zy?‹/ÚºÖh?ï$ï΄ˆ?/ߧ×F?aÿP7
?/ߧ×F?ï©Ì"Ió‹?fÝÝîî—Æ?…ŒÞê(?fÝÝîî—Æ?ïö0¯—ª?WŽny¤–?SǞFü9?WŽny¤–?î'ùŸF?¼BM—ãa?®ގ®=œ?¼BM—ãa?íÓiB‰?¢ŒÓ_#-?±dµî™8;?¢ŒÓ_#-?îÊKGs~t?"'là2Ÿ?£[K‡J¾?"'là2ŸAGN3FGL J1725.0+1152@A£_ëøâ@8|H 'ÁçÀ7ì=s(À:½ ùt˄?îJh[´×@…¬àa?þ*?›Ü?¿æë'Éý¿ÞÓÔmÕñd¿Õîqsp÷¿×e:´SP¬AGNbll@§í§¯·éPowerLaw1H 1720+117?ïþµ€çh?"McìcOž?$§í¥(X˜?"McìcOž?ïyŠ"þ`T?¬éE¡œ]É?Î­‡-z?¬éE¡œ]É?ïx"âAög?Ê—‰;y?íƒ°áû+?Ê—‰;y?¬é?rVÖ>þ%?[ù'V&?rVÖ>þ%?ïüuÙéA?9}¤Û?<Q6S¿'>?9}¤Û?í@§ø#Š?À:Íu-?µúÀ>ÈW?À:Íu-?ï=³…?'œQM?¸0¿'ºÅ?'œQM?îk–Q½?"3sÖÚ?¯IF™762?"3sÖÚAGN3FGL J1725.1-2832@v^"@lÚ@û6à÷IÀ8·N?(3üÀ:†–UAzõ?ó³'6{@;e[Ï_@Ìõ U p¿äÀ€æDm¿î¿'Þt†¿Ø+¸ëny¿¼Ç5oùbOTHERspp@ˆ''Á"³§PowerLaw?ïA¯?s2}?'ÑaNR?—ÊrFr?'ÑaNR?îàf;Ë?³@ÿ8U?¡þ©Ÿ¾OE?³@ÿ8U?ì˨fՒ?§3aâ`Ae?¹¢¼ÌSp?§3aâ`Ae?ï|dš^e'?xîltø?sl´3Mà?xîltø?îv†:}e˜?¬hèçS™'?¨—œSÞ#Œ?¬hèçS™'?å†[rÜ/Z?Ñ+LÑâ,Ó?ÔóIG¡L?Ñ+LÑâ,Ó?êŒM´Fw?¯Ã§"§?ljÎÉ.æ%?¯Ã§"§?íêŠÃ
õ?¤±Käp\¨?°«©èKwZ?¤±Käp\¨AGN3FGL J1725.3+5853@Ußϟåãõ@@ÿŠßÂr×À:cµ±þÀ;ïLñJZ—¿éù@ö#Ÿ†)@no?þȝ¿á ÁCà28¿à«¥Îö¿ä/vve¿ãñÍhAGNbll@š"Ô`ªdÃPowerLaw7C 1724+5854?ïÿžØë
?–7Zd¥?I¶B@d?–7Zd¥?ïØ?›½E?†b	L~?sà2‰¯á™?†b	L~?ïñr²é»Š?_y>j&ïî?]š¢»{Ì?_y>j&ïî?ïÿxMnž?	ÆÀoÜ?Ðýw¤,?	ÆÀoÜ?ïÿ_VQÆF?ç¯óžk?0şû?ç¯óžk?ïC	ȉO?ªhÿP‹;?œžÍÎ?ªhÿP‹;?ïäÊ3â§ø?u ;Å1=?k5Ì>TH?u ;Å1=?ïñ«¬?V]ãVmGF?]ܨì)ªº?V]ãVmGFAGN3FGL J1727.1+4531@Q܇ Q»@@©÷¿¿žÀ8¢Ëlz|žÀ;¯ß´tç?õ`]æe$G@{bcL@¡\3\£Å¿äZÇ´Š
Û¿æƒÿíFâ¿émKŽ¿ïÿ{z
§AGNfsrq@tÑ0#̎LogParabolaS4 1726+45?ï÷"C:¬?J8ÅwpÙ?Pý»?Ñ8,?J8ÅwpÙ?ï¹+¸?¢?‰-ž	E?µ￉¤?‰-ž	E?ï+%ž'Ñ^?Œ´_ŽH?š›LAå;?Œ´_ŽH?ï2ÿ³BÑÑ?z8{	t<¥?™ 	"6)ô?z8{	t<¥?ïöŸþ|a?R¨¤+ÊZk?RÀ-¹y?R¨¤+ÊZk?î-²&¡?¸v¨>?¯}$à2zê?¸v¨>?ïŸjþ&?—8ë'-?Œ;7A=?—8ë'-?ìß]5?§v®Ñç?¹½Õð?§v®ÑçAGN3FGL J1728.0-4606@uy¬¿±[WÀ
€F6pÀ9:¬.Ǔ¨À:üº·÷R²?ÖQœˆj@
×i0EB)@x?V×þ¿éÀ	oëJ¿ß<Zú!™®¿àeýö:"`¿ìÁ°~ã_áOTHERspp@™ýDg8~PowerLaw?äêEV~ðT?Ë
˜¼Fd?Ö+uSY?Ë
˜¼Fd?îûã+Åý?ªlxW¸JJ? AÍFB¥.?ªlxW¸JJ?ç±7ñð?²ˆñRS?НùÎ?²ˆñRS?îç•ìÍ?"ÒvŠøW?£Å†¤¢ËÂ?"ÒvŠøW?ÌÀÄK"?É]é¦]‰?èÏÎí8}?É]é¦]‰?ãñ$¶K^¬?ÍâR¬0†A?ض"iB©?ÍâR¬0†A?á_¸#a¢?¼­©Ü\â¯?Ý@¹é<¼?¼­©Ü\â¯?æ)_ö­Ï?µýñ"}'×?Ó­Aü¤a?µýñ"}'×MIXED3FGL J1728.0+1217@Anž i—s@7þγ#®À9u;â.]áÀ;= 8Ûê¿å´ñÙ÷'®@ï¼C͈@@w˜¿ÓNŸ~ú ´¿æ¬Ó;ë'^¿ã¦®Å¿é ›Žf_°AGNfsrq@"û 'RTaPowerLawPKS 1725+123?ïûö)¬: ?Pß÷`B	¹?@'XSK»¬?Pß÷`B	¹?ï´OÍó"`?™!pt#–È?'ì‹Aï?™!pt#–È?ïN€…÷P?'óÔ¦õr"?–=ÏïAõ?'óÔ¦õr"?ïÿ/ˆXԂ?nUÉÅÎ?ñ˜!ºœ?nUÉÅÎ?ïþžʬ?2@ÈÕÕoO?&ä…B2?2@ÈÕÕoO?îR	)ÊSÌ?··ëö"À?ªßmd6ªD?··ëö"À?ï¡7%cÅ?•6¸C¨Ì?œëÙtO_?•6¸C¨Ì?ïø,c±f?GW"|ÔZî?OOÂÖîՆ?GW"|ÔZîAGN3FGL J1728.3+5013@SE@€"Ð@@ÃF߸aÜÀ9!EºtÀ;~JÏ1+¿ü=¯
@ìuN‹©A?ÿ[–~²­¿áÛ0–†ûÿâ*"Ô€Þ¿ÖmæÚ·i¿â$í|ÓAGNbll@Ÿv_Ø­¬PowerLawI Zw 187?ïýêâ£?*óÇ®(¦0?3©ÎÖQ5?*óÇ®(¦0?ïâFA`{?|ã&´?m¹¾¦êŽ?|ã&´?ïÝXûÓö?p¦si} Ö?qS°íx\ì?p¦si} Ö?ïÿíÆ->à˜"¶ºö%>â9ûQeñq>à˜"¶ºö%?ïûÚFn5?:"®äœu#?Aø–……a1?:"®äœu#?îûCè.Ÿr?±ãùR%ŒŽ? KÁ~ÍÖÜ?±ãùR%ŒŽ?ïÈÂQÔÒ?lµeˉ?{ž×{djÝ?lµeˉ?ïþ¡
²?(Yú¸!â?%ï\Y>x@?(Yú¸!âAGN3FGL J1728.5+0428@;W¿PãG@4sÔ Ö¤½À8îdüÀ;Cí\M?òˆB+ž"U@Ɉ$Ì@ÀÿÿÕâ¿ä«ZÌ ÌÌ¿çÒ{•w ö¿é"i+üÄ¿ïúÊ;ÅJAGNfsrq@AÿàŠï³PowerLawPKS 1725+044?ïô¤ÐhÊ?RâíÁÖ ù?V·àu+ì9?RâíÁÖ ù?ê{P)§Ýï?Â(²]ñ"?Æ¿Y`ˆE?Â(²]ñ"?îðË«JØ'?"ñbI? óEJv––?"ñbI?êph•7,?Ÿ?¶Û;(	?ÇÒ>]«#Q?Ÿ?¶Û;(	?ïíT|â‡R?møéNX?b«ƒS•ê?møéNX?Þ#q:; y?ϙ DÙxØ?àîGbâoÄ?ϙ DÙxØ?î+ß]Y]¦?¢Š)MnW?­B
*j%§?¢Š)MnW?ÖúA&]Y?±cÒÂ*•?äž"ßlÑS?±cÒÂ*•MIXED3FGL J1729.5-2824@vhË@p2˜@
!ç@–sÀ8ÛwˆÍ™{À:¬¦]¨R?üó…†QŒ@^köÝ@RtÈ©Òw¿ÊÃõùó¿êÄȼœÓá¿ìd1Xh¿ïþûB0&OTHERspp@"UæffffLogParabola	?¯†Ü¹»?Æ}.Çò%*?ëTHё>?Æ}.Çò%*?¬D#½Á¹k?Àg'Õ È?î;½Ä#äi?Àg'Õ È?ÙÀ6çGÍI?³·v²xˆ‰?ãäŒ\[?³·v²xˆ‰?Á®°ÿ#¦?¡¦÷´®¨1?ë"Sù@7?¡¦÷´®¨1?¦²òÙlf‡?¯´ÐPÁ·¼?î"ÐÒ?þH?¯´ÐPÁ·¼?'—hõu?­ÆöHAk?ïo#GòvÄ?­ÆöHAk?ÓØ ¥3x?¸ŽúÖ¶µ¨?æï­fCñ?¸ŽúÖ¶µ¨?s¿3iá[?'Á0L|?ïŠ1$š?'Á0L|PSR3FGL J1730.5+0023@7ÄÊÿm3	@2-ß6[ÝÀ8Aðþ}=À;ÅJøK×?𭷀µG@×6aæÏØ@ƒ@7'´¿ßùnurý¿âh!š*¿âqõvlÌe¿æ'>×+KAGNfsrq@'Ë·XâPowerLawPKS 1728+004?ïþê€*Ìv?·UiJ?!XZ$œ?·UiJ?ïo³"›z3?ªÍ2ܟs?'	›£ù³¤?ªÍ2ܟs?ï¢BN'?…aQG©	?‡{ïp­ëu?…aQG©	?ïóá5ki??kl"{Ÿš?X=õ!¶NR??kl"{Ÿš?ïþ*°?1ÒÀä¦Ì?/®ÇêӘ2?1ÒÀä¦Ì?í[Xbºå?ÃRdÚRÏä?µ%<ëçÆØ?ÃRdÚRÏä?ïL#¿†q?'Ò{º÷$?–{1æ?'Ò{º÷$?ïäǪ5?aõ¨ÿŒ>r?k8ðâUË?aõ¨ÿŒ>rAGN3FGL J1730.6+3711@Né"åx•@?\
ÿ7ƒ$À:p¨ß‡ºÀ;ÐaP?í±½k[@yò'>N@³À€8Iž?ëQႢ˜W¿å˜tÄ´5¸¿ÛIlΒþ(¿æüŋÃu¿AGNbll@›Mâe,PowerLawGB6 J1730+3714?ïý©Úô?7Ž¡¨…â§?7'³BeÔ?7Ž¡¨…â§?ïQõ/k? —	JÆ;¨?žõÁ`þŠ™? —	JÆ;¨?ï¿Püƒ?{•Š+j¤}?€+ÀëEi?{•Š+j¤}?í»Ú\év7?'|øê?²!-ü€K?'|øê?ïû¹¢'e?FÃüS7$?AuÊX#?FÃüS7$?éöä³s_s?ÅÞ.[j›?È$m22'3?ÅÞ.[j›?îÔ&w°]"? IIs\0<?¢½˜Š'æ? IIs\0<?ç;FlöÎS?´ŠØh?щs&cZ?´ŠØhAGN3FGL J1731.8-3001@vW¼ ?ÿC^¿S À8~ŽŠqÞjÀ:…‡ú4ää?ðD%'_
'@
®>lL?ÿÅ*A*¿åf?²ûóß¿ÊKf»uâZ¿âD˜L׿á6g\IpÑAGNbll@².1hr°!PowerLawNVSS J173146-300309?ûÖ¶Â?žŒG*ô»Í?ˆ"{£?žŒG*ô»Í?íooÕâ?¸¸—«³?´"Q]Dž?¸¸—«³?ì—%Zô?¨Ä*5˜?¹ëF×Í(_?¨Ä*5˜?ìÚ{"c?')I¤?¹/¼$®Â?')I¤?îaO–ì?§âýÐJ¼¯?©î;'>¬?§âýÐJ¼¯?ÕÐ6»Ë?%?ˆR®½\?åä¢`m?ˆR®½\?錙"r¾?±°²CÚVj?É͛v5ì?±°²CÚVj?áUé6öóM?°ƒ^—œ?ÝT-'f?°ƒ^—œMIXED3FGL J1732.5-3130@vDüÀz®ó?ð?8?®ŠÀ6 ?û˜'3À:3X–š@
u9ó–»@FÿÙ> $?ëÊS0‡9ù?ïÿ(#,!¿ÂwÕRò.¿äƒÊ'´'‡¿î3&‹ÉPSRPSR@™'ð‰ 'RPLExpCutoffLAT PSR J1732-3131?¡¸ï¥D'?»¦uààj?îäq
.Ø?»¦uààj?è õ?¹J=[˜;§?ï¿jäzh?¹J=[˜;§?²£›;p*?¤­·Šzª²?í«Œ˜ª0k?¤­·Šzª²?KxF-£C??¨÷þƒB?ïù!Ûá¬r??¨÷þƒB?À­3Œeæ?Í<
a½?ëÔ³Üæ‡?Í<
a½?€¢9iU^?}õA?ï½w6"?}õA?ļ‰Yk½O?·Ař¾Õ?êÐÝ©¥¬?·Ař¾Õ?/Ú-ÔÎ>?1}ÁD2ݞ?ïþ]c™"?1}ÁD2ݞPSR3FGL J1732.5-5048@u@i³únÀ"ÖÃà'TÀ9}:í;ØÀ;W
V›H?ÔÂS*ä@$QËú"Ü@Fk€V§'¿è¹?H·¡¿Ýqtºf³¿èú4È«ø¿ìê×ýêPSRPSR@Ø©*0U2PowerLawPSR J1732-5049?ì.°Þô[v?¼L|^ºs?¾Šy]$Q?¼L|^ºs?ïo#Œ]? /=*9Ö?'ŸyÖ¦W? /=*9Ö?ëS‰ófó?¬jû׎?±Ø2d3å?¬jû׎?ï\šD[Æó?u!sûÌÕá?"l·wö½©?u!sûÌÕá?åaqz@¹?ËíÊô/'??Õ=~Ž?ËíÊô/'??êåÒÚØÔ?ÁÍ~ŠË?Äh´"œ¯¤?ÁÍ~ŠË?çw öZ:?¸ÀtHk•?ÑÕ¾KŒ?¸ÀtHk•?éb"Çø§œ?®Éz÷‡?Êu¬àa?®Éz÷‡AGN3FGL J1733.0-1305@(÷ÞÉN"@% 6^`ÞgÀ7'ÎuCxüÀ:¸M`Ûâê?õ5ÁB€D@Ç2]Ë7K@éð»>"ö¿ân¿«œë¿æ'Åeòš‰¿ä­cÐß׿è*»¾—ˆAGNFSRQ@€"·´¢3œLogParabolaPKS 1730-13?ïúîk¶ý?WÂæ[t‰?DFP"9T?WÂæ[t‰?ïkIÈ{?¦•'êg?'öÕǸµ?¦•'êg?ï1L•)?–è¥EtSd?™Ö}-Zߨ?–è¥EtSd?ïþ‰ý^(ï?ßAHèÑ"?'`(MrŸ›?ßAHèÑ"?ïøêÈÙ?Qû¤Xëв?OèT¶0Žk?Qû¤Xëв?ìãö»nç¥?Äëxù
{?¸àJ%ҝR?Äëxù
{?îi¶¸
x? ‹ë#"?©d"|"Ê)? ‹ë#"?ïþp‰]"ä?&X—öË0½?(÷hPr´?&X—öË0½AGN3FGL J1734.3+3858@P"ÿÖåU@?…_Oñ°À8GuÇ,yÜÀ;m>m#
?ï6¨ê¼@]®:æ[@€…Zmà¿áj0]Égp¿å­è…ù¡¿ãÁ5,»''¿ë_š‰ŽAGNfsrq@…÷½¥PowerLawB2 1732+38A?ïüS_oô|?6o*"Š?=ev¦"»?6o*"Š?ï×Q¿ ¢ô?'ü$@¸•%?tW nþš?'ü$@¸•%?ïÏ×?ƒnÿï?‹úLBëæW?ƒnÿï?ïþ4Æ'¹z?
eÖ	a?,³ iz"ÿ?
eÖ	a?ïøÓÚ÷̚?Lcvg
?L°"äá6à?Lcvg
?î×èí§?±_Ōƒd?¢àI§?±_Ōƒd?îžÂ+šHÒ?œ)¾¼Õ
,?¦ÝCǽà?œ)¾¼Õ
,?ïüàc, ?6M©v?8üærPŒ`?6M©vAGN3FGL J1735.4-1118@+Æ!à$˜f@&sA¿½ð'À9OsGö8×À;4žm>¿êšŽÇ-¦@ç\20@@O¿Û͜¿Ððs{ÞÙÑ¿ëºeð°èҿΤf/0¿ØøáÎ;·¼AGNbcu@¦¥7Ûô‡ýPowerLawPMN J1735-1117?ïùzLCÇÍ?Kùš2hR?JÍóýŒ?Kùš2hR?ïqRr過?§Ôãûö,®?'Õ±©¯*?§Ôãûö,®?ïƒàøRâ{?ˆ/çI0è¯?Áç×ÅB?ˆ/çI0è¯?ïÿƒ"ô	ì?yÿ["B?Έ y?yÿ["B?ïðc$	!?`WiÍyC?_9·¦[ß#?`WiÍyC?í/¸#"Ò?êY£Õ?¶'>á¡¡ú?êY£Õ?ï,ϟm¢?•ù&òށ?œšfñƒÂ?•ù&òށ?ïüwŽ›¨?5I!òñà?<CŒ_dÀW?5I!òñàAGN3FGL J1736.0+2033@F@L j@9k>¿XpÀ9rêUrùÀ;P…Ûv³¼?ð%ä‹Zf©@sòoɑ"?ûŒ@ Y&b?ïþI™HˆQ?à6¦,Wª¿Ø^~ŽXüN¿×–fUÁÊÞAGNbcu@²	¿;dZPowerLawNVSS J173605+203301?ïòn4;	?[è
ÔÍ¢?[#—¨} ?[è
ÔÍ¢?ï&JQ)_Â?³›a]ғí?›6µÒ=Ç?³›a]ғí?ïZ3†PwÎ?ð"3E€&?"¹9`¢A?ð"3E€&?ïû"<²…?'‰t2Ýe?@v±áZ?'‰t2Ýe?ïÞ½Dfá?r$F›™ÈÄ?p¡]Ɏó±?r$F›™ÈÄ?ìÐËUîý?¢çh0?¹y¥RGf?¢çh0?îm3DP? ÝQ'°‹2?©,˾n‹? ÝQ'°‹2?큆‡z?¤ÐAû'Ë?³óËÄÆ
i?¤ÐAû'ËAGN3FGL J1736.2-4444@u˜¨ÙºÀïLßזÀ8ZHùn‡À;S‹'?ó1£™D_@ˑô^·@'`gÁ¿å±öy|Ä¿àÀЪ§Þ׿æMÞzt:d¿ï#û½{ 2OTHERglc@‰×çæšÔPowerLawNGC 6388?º†Dt›Å?¼×òÎFÓ?ì¯7ql?¼×òÎFÓ?ÀqÇ÷³í?Å7o§qP?ëãŽ?S?Å7o§qP?ãeQÇs?²ñPÌ·ƒX?Ù5Ã\q×?²ñPÌ·ƒX?Ô¼PчOH?¬Žªð\ˆ'?å¡×—<X\?¬Žªð\ˆ'?€ïjúÑô?'ØQ'tj?ï¼BW'6À?'ØQ'tj?™ˆ¼Ã
ˆ?²D`Ckøg?ï3ºõR0?²D`Ckøg?ÂÕso8r?­°uæýsµ?ëJ£$1ã}?­°uæýsµ?¢éþQxD?ŒUãcfƒ?îÞA`6e\?ŒUãcfƒMIXED3FGL J1736.4+0634@>EÑ q$0@3¤:?–îÄÀ9 QJuoÀ;G›	b@?í10âKF@êßp"eù@فà?pX¿è'%xyR@¿é
ÎM$¿è@doÒ\¿ïþ÷‰[U^AGNfsrq@|qQÕQ×PowerLawMG1 J173624+0632?ïùé}²ˆS?DU&úŽj?HZ‹þÑä?DU&úŽj?îèSÈÌY'?¢Ê'Ï
'??¡zÃr^€å?¢Ê'Ï
'??ïQÔW÷Ÿ?"ó2°"×?•Åu‰>?"ó2°"×?íðͱ_o8?‹Õð<1—N?°y'uàmC?‹Õð<1—N?ïøƒ¡hN?LŠ¿g{àÔ?Nðƒ‡§?LŠ¿g{àÔ?èô$Cp?Êj+Wq«ê?Ïà/nò?è?Êj+Wq«ê?îùù‡&5°?–‰ú•2Ù? `g'@ü?–‰ú•2Ù?äã‰{®
?´B"¦Ð?Ö8í£ßæ?´B"¦ÐAGN3FGL J1737.3-3214c@vD*Ÿ{Zê¿Ï*À1äÀ8kógkI$À:|Oø?óÁwO>'@'ˆíNø@$H¿aL¿È4ì›Ê u¿è6U'Ìc¿áȵ¥8¿æÕožŒÙOTHERspp@ª#Ò£S&PowerLaw$?ãŸS‡¹¦?Ñ5ºô2A?ØÁYÐðŒ´?Ñ5ºô2A?ëR
p¤á?Âì+YA‡+?·›Ö=l{?Âì+YA‡+?ä6O¬Tv?¶#€x5pÐ?ד`§WÚ?¶#€x5pÐ?ëÚúºWh?šo"t4Šj?À"¶¢`?šo"t4Šj?Õ)Qÿ7i_?Ìÿ|yš˜?åkWdKQ?Ìÿ|yš˜?ҍ°à» ?ɤÜî­ó?æû¹'¢0?ɤÜî­ó?â=Kmš?å?·I¦Üá?ۅi$ˀ5?·I¦Üá?á z]X¤?µ Ð¡Ùß#?Ü¿EOâ¹?µ Ð¡Ùß#MIXED3FGL J1739.0+8716@^Þ˜¯@;ñ¢@1HwÀ9§~b®–À;Ýî­È$Ç¿óÅΞ^$y@r6xâêÆ@7ø¿Äс¿ÔcÏÁ&"¿çÕ¬A3sl¿Ü
û˜/ë¿åŽ¨ê¢ÿAGNbcu@'	ýŠÚ¹õPowerLawNVSS J173722+871744?ïÿۜÀ·ã>ù~¼ì§5f>ò1¿lqUH>ù~¼ì§5f?ïß{ÜÖkm?ƒ‰Z™Â÷?pB¦¨AC?ƒ‰Z™Â÷?ïáѼ
ô?q"겊#?n.=F±¼?q"겊#?ïÿÿÑr›>"8z$žAâ>ŸB²qÒg>"8z$žAâ?ïÿ˦gŒ>úaýwF>ú-²€9y>úaýwF?ïG¡S̜?­#æþÓå?—Չ$zŠ?­#æþÓå?ïÉaƨ˜?€öÿ¤ÞÍ?{O÷OÉ?€öÿ¤ÞÍ?ïÿû3<J>IJSk|P>Ã2ôÑÎÉ>IJSk|PAGN3FGL J1739.4+4955@S8ß¿î—ù@?¹´VÝ\À8à±é·ìÀ;¨Üôb=¿½EÄh@9¿ím@tÔÿ÷«¿ã68š6ˆ¹¿ãG×æÂ}z¿èÈ¿%璘¿Û¢'ĹAGNfsrq@‰¤u?|í'PowerLawS4 1738+49?ïÿVk‹X'?C*>½Ï™?2Š«üJ?C*>½Ï™?ïÛN¯e‰?,j!؛?rؾJ»?,j!؛?ïÆêüýZù?xÆÔŽØ?|ŠŸd?xÆÔŽØ?ïÿò*Ì©´>͆¨‹_ü>ÛªÈKZ£>͆¨‹_ü?ïüáO0{?;©£ºÜÓC?8÷Öòl_‡?;©£ºÜÓC?ï˜Öƒ¸d?°iýÆ4?Ÿå6h+i?°iýÆ4?ï;EªwB?"	¡É¦Ã?˜—J¸I­Õ?"	¡É¦Ã?ïÿČȌ>ÿ#â;ÇÃÝ>ý¹¸¤Çl	>ÿ#â;ÇÃÝAGN3FGL J1740.3+5211@Sム3Ï@?Ê.Íû¡À8|6™AÀ;¢¡€è?íú9wEï@Úæ1ø @ž¿\V˜¿â@þŽ`¿ç%ÇçØ
j¿é¥Oê<ãû¿ßÃì]$¸
AGNfsrq@#+JPowerLaw4C +51.37?ïÿ‡AН?
)t;Ëãz?/·`ý¯Ó?
)t;Ëãz?ïÚ/
´žƒ?ƒýQéótd?rèy+à
œ?ƒýQéótd?ïĖI¥\é?z)À¼ÏA?}´ÛûÒ?z)À¼ÏA?ïÿ(¥e«?	Kôv?šäDgt?	Kôv?ïþЁˆ?,-ýðâ,Å?"÷ìAƒI%?,-ýðâ,Å?ïmå`Âc?¯åÝ6sÑÖ?žòCY§?¯åÝ6sÑÖ?ïƒ}Ýó³
?™~¾7bâ? ˆ†'Ø»?™~¾7bâ?ïýËõXÔz?/x:8£_"?1 UÏþCT?/x:8£_"AGN3FGL J1740.3+4736@RÀ'¢Ü@?SÂÀ®À:gø[ÆÐ4À;ìP->ýl¿ðÑÝgú*@攸‰Hé?ÿ&Šþøï?çâQ]¸q¿Ù£»vc3¬¿ÛúS0‡9ù¿ßþ«íŸðAGNfsrq@¬-æšÔ,=PowerLawS4 1738+47?ïÿ	—GH®?¸ý«õŽ?ÍÈÕ¡?¸ý«õŽ?ïÒþž<QÑ?ˆ‹Ý9´ß?v€°á'+w?ˆ‹Ý9´ß?ïà}½´Å´?a7¡>òa?o'B(Þ4m?a7¡>òa?ïÿŽt2½ÿ>ÿ>yBÞ?bë2Ý>>ÿ>yBÞ?ïý¢ð°VÊ?0MHK]ø_?2è{yqÐ?0MHK]ø_?îó֞T5Ú?±"¿v‹j? Â–PWb?±"¿v‹j?ï­¼äwcd?ƒf‰‡Ý£?"Æïå–ø?ƒf‰‡Ý£?ïúŒªâ?Dw¹Ð2'?E͈Öÿæ'?Dw¹Ð2'AGN3FGL J1740.4+5347@T[O?Ù3ã@?ã$H¸À:h\ïÅYÀ;÷Ÿ<pÊ¿ç¾W¢:@
ƍ³\cX@&"_ ¤{¿ì¶ø–‡™¿ÝKH·Ì,¿Ðú&2ë.¿àÎ[‹Ó§AGNbcu@§§¯·éPowerLawNVSS J174036+534623?ïÿ)Æ¢ç ?;%lm…?Ç)ÞHœ?;%lm…?ïÕÖ%»üE?‰=Çô'[?uí.`uj?‰=Çô'[?ï塛âT?jEäË"&?j^dŠ|Cë?jEäË"&?ïþX'8©?>…œÜ÷?*vÜPÞt×?>…œÜ÷?ïþ*A¿_s?%Åÿ¬v&?-[åyEoq?%Åÿ¬v&?îô8R,º?«Ék[}0+? ¼zß¹g?«Ék[}0+?ïÒûÐùàµ?zH–ù—?v'–ýa…?zH–ù—?ïì"–ÝI?^hW1š£?ckërÁžß?^hW1š£AGN3FGL J1741.1-3053@v]:à;>š¿ÊUNÀFExÀ7â¸ø²<À:Ò³–šâ@Kڞòt@ý¸§ü´?ôdÐvû_?ä-v€dê:¿ÝW¯¿JÙ¿å–œ>‡È¿ît>ág8žOTHERsnr@>²{²þÅLogParabolaMSH 17-39?bÉ)ôUõ?{ô>Ò2ó?ïí6Ö*[?{ô>Ò2ó?² ÑÅ?Àtâ4èêæ?í¿ÛåÄj~?Àtâ4èêæ?±èåQ}öü?¥&6"þ*^?íÂãU‹ˆñ?¥&6"þ*^?É<ÈE²v?©ÆÓ¹yT?é°Íî"y£?©ÆÓ¹yT?j¿N¥ «²?"ªÖ,òÒE?ïå@±†ý?"ªÖ,òÒE?•äk'Ôõ?¬ÄRAûª?ïPÜ£¦Û?¬ÄRAûª?§ß`ˆŒô?¯n¤cÒ+i?î'	÷irN?¯n¤cÒ+i?¨í™¦"Ì°?˜"Êw8Ž?îq&efÙu?˜"Êw8ŽPSR3FGL J1741.5+1351@Bð¾@Bo@5¢Àu¦uÀ9äêÅX/À;'H¸?ñÁ˜H¶¨@"—G…@Í,@zÄl?êÕû]·t¿Ü6]`¤0¿æþ5¹['¿ê
.Ž€-YPSRPSR@"VuY³Ð}PowerLawPSR J1741+1351?鎸yN?Çq•ëlÔ?ÉÅžÊÆ?Çq•ëlÔ?ä÷Ó>èp?ËÜ*«Ø¾ü?ÖY'/ù ?ËÜ*«Ø¾ü?ë ð7àìê?¬Å³ÕQ?Á|? |LW?¬Å³ÕQ?ç3ÒJæ;?¨¸1ŒÏb¨?ј[jx³Š?¨¸1ŒÏb¨?ÛÝ Úß=?Ò:læËÈ?âoÀb?Ò:læËÈ?Õs)]F'?ÐÅÖ°È­?åFkQ\¾ó?ÐÅÖ°È­?Ùåv€©¢?Ã7e‹¹ËØ?ã}
D¿«/?Ã7e‹¹ËØ?ÐȽ@	QÛ?µ)Ò©8?盡_ûW?µ)Ò©8MIXED3FGL J1741.9-2539@ÚÜ QÚ@XÀŸ—à\À8µlC9À:m}F|¼¿¥²ŽÙ³KX@
ש`Œß@¥@¿ ?é>ˆÅ{¿à0àÍàž¿çÖësd¿Õ¸ÁÀ»AGNbcu@¦#S÷ÎÙPowerLawNVSS J174154-253743?í9ã KO	?½m†øút?¶0æþïb8?½m†øút?îä[ Ôe6?¼ãAÊ8b?¡ºEñÝŜ?¼ãAÊ8b?éDi­SñÖ?±#ât3L?ÊîYJ°8©?±#ât3L?ïí4NY??T*nîì –?b˱Ô)á›?T*nîì –?äC'†!d ?Í·—õ™d?×xÚó½7À?Í·—õ™d?ìr"wÿ§?ŽxË1°ì?¼nïÄ@Ç?ŽxË1°ì?èõÃVŠ?´#õ-J-N?Ì(ò¥×óû?´#õ-J-N?ï@¨¨;"!?'ö™mÝz°?—êêõßì?'ö™mÝz°AGN3FGL J1741.9-2054@¨u€4ì@˜ F†øÀ6Û¸KgÝÀ:˜ùN59@	ÈWQölÙ@°5<wÕ?ü&µü¦¯,¿Ñ½Zý/HË¿ã:*k¹b¿í2äÝÿhð¿ïwÅiÆPSRPSR@…֌篸PLExpCutoffLAT PSR J1741-2054?LæËX×?QŸ†Pc0+?ïøøan?QŸ†Pc0+?ªÕÐéÓH?Ä_'©_½?îR®Âºi?Ä_'©_½?¨ç;͆g?Ÿ2¥L]Ú.?î~ьz!Y?Ÿ2¥L]Ú.?)­
¯Ás?òÃt̳?ïþe.¿g?òÃt̳?BÍG£ëñ?VE‰e[?ïûL®s4D?VE‰e[?'ôtɐJ?´{	ùÖ?ïh\Yêy}?´{	ùÖ?‹¶y0	?í¨è« ?ï'&PF?í¨è« >õ"¤ã+™>òËÙNj¿?ïÿÕÀ¼HE>òËÙNj¿PSR3FGL J1742.2+5947@V àè@?Ï¡àø0À9õ@UZ¥hÀ;ë½¼Ž'(¿Ç®ö£
@ÕáWHfK@hÆÿ®K'¿êН<¿ämtkH¾¿Ütû'毿áZ3RÆTAGNbll@"py	k¹ŒPowerLawRGB J1742+597?ïÿ"l"ö?Òi0ˆäd?
åØԚ?Òi0ˆäd?ïØDÏÈl?ƒ¬'Î?sݘf.®L?ƒ¬'Î?ïã)†NÁ?|4H"B¸>?lÖy:ÕÇ#?|4H"B¸>?ïûÓz]`¦?&¥ƒŸäÜæ?@²Gø,é?&¥ƒŸäÜæ?ïÿåóºL?¬Í:/?†…š"¸`?¬Í:/?ï-Lþ¥%Ù?¦ýT˜ÍZ«?šV`)£vï?¦ýT˜ÍZ«?﵉áY"?†LoXù!‡?'‡¨ëó	?†LoXù!‡?ïÚAâDû?gd'®d<?rßDŽÀš?gd'®d<AGN3FGL J1743.9+1934@EêG@0q¸@7Wà0VàÀ9ŽÊƒ*ÂÀ;Z´Î©Eß?ÜýÐö…¶@
(w¹õڍ?ünJ 	µ¶¿à'󆹱׿ÐláÈ¿]¿ÍíÖèY›'¿á"'¶®"AGNbll@¯7[À6ãPowerLawS3 1741+19?ï÷SpëOš?V?#å¹	?QY»mM?V?#å¹	?ïŠÞŒþè?¤¸°açc—?HÏÖ%?¤¸°açc—?ï£ÇŠÃ'ç?'ÿKн
 ?‡A\Ö@?'ÿKн
 ?ï|åŒiãÒ?r8—gºuD?cN{Z‹´?r8—gºuD?ï§O7©B7?†È$erÈ
?†,2M?†È$erÈ
?셇éÃÓ?ÄLé›BCÐ?»ÓÀ±ád	?ÄLé›BCÐ?îÌwý½…‡?›ÌQDÈI?£8€ ¸"?›ÌQDÈI?í$⬡Íß?¤´ÿÒb×É?¶Øê™9Ã?¤´ÿÒb×ÉAGN3FGL J1744.3-0353@5"?·¥ô@*
N wmÀ9œ}¬ðÀ;ŸÑß[¿Éw"\‡{›@
>µÿUá@'WÀ0\>?å#Û´ÇŠ¿åcÊøÒæ¿â݇®úBÁ¿æJ~É0õAGNfsrq@Ÿ1Á½¥PowerLawPKS 1741-03?ïòûI%ґ?je˜½¨ûã?Z	m}aµ?je˜½¨ûã?ï]{ü¶Ü?²[)ˆ™Ôî?"OЀi$?²[)ˆ™Ôî?ïN7tÐ%a?‹Á¯Õs¤?–9eûSë?‹Á¯Õs¤?ïå¯9òr¬?RþÃ±Gò?jPÅö/ûÓ?RþÃ±Gò?ïùæDž÷?H¬÷WUu?Œ†Týº)?H¬÷WUu?ìÀ3ÕM,Œ?ÄÔ`õŽ7?¹þaU–›Ÿ?ÄÔ`õŽ7?í;"²K[?©º0p"Äv?¶&êkf#?©º0p"Äv?îõk
©Àó?'±@ž8ŒO? ©ORÐ;Õ?'±@ž8ŒOAGN3FGL J1744.5-1133@-¦C?ñC@"^C ÚxÀ7ö›ÅÃÄÀ:Ùxà¼mÚ@.Ħ7¸@Øâ'q	@'¨ëF4˜¿ÙÉñÛÏôõ¿àÚz5Œe¿ê£Ö0Ωò¿ìÀ"•W¿PSRPSR@‡|kíúCþPLExpCutoffPSR J1744-1134?dƒÜ'»?hP>Œý²?ïëÿûMh¿?hP>Œý²?§(î?F
—?¿Ð?™¯$W?îq]—?¿Ð?™¯$W?»`
`)¥/?¦ÿP§",h?ì"þSúËZ?¦ÿP§",h?"Ž'RÎ.!?{"Ó»™=½?ï[‹u®F¿?{"Ó»™=½?YwwÕ'zõ?Uòԁͤ&?ïóDDAgB?Uòԁͤ&?—r?¹UB¸Z{¬?ïDo;»€?¹UB¸Z{¬?—§Ÿo04\?"ïñÛÈ?ïBÃ]C
?"ïñÛÈ?bßÓM'Í?T#Ý`àî×?ïí ,£Õ?T#Ý`àî×PSR3FGL J1744.9-1725@#×Àâ¯@^á¿Î¼À8Å]Ó6À:ä9]ßË¿³»ëñ-¾Ð@9òj@›Ä?àj¹¿éùrû¨µõ¿á
ąšM
¿âÛ¼…¿×yµAڄµAGNbcu@§àÝ<64PowerLaw1RXS J174459.5-172640?ï÷*×+ö?Pèïòޅº?QªRàã®?Pèïòޅº?ïáqZÇ]?µ'…/¶CL?œãÑÙÎ~X?µ'…/¶CL?ï•ös(/Ž?‡¾6ÐÚJ$?Š'c/ä•?‡¾6ÐÚJ$?ïø`_¢c(?9 »{,™?N~€¸<4@?9 »{,™?ïÚ*úK,?sL.;X™ë?rêƒH&$?sL.;X™ë?ìKÒû?Æhò¡Œq?¿U§Qh'‡?Æhò¡Œq?ïh?Y‡0?–,},=°?'øfø?–,},=°?ï°´·=¤?x÷p§{í?ƒÒÒ.èI ?x÷p§{íAGN3FGL J1745.1-3011@vmú WŽ\¿â…'€ã"À73	~.IÀ9ºrW5q@æ|®§GØ@[Yèÿˆ?üÂHÊt,ù¿âáê ó*/¿ã"±_ÞâÏ¿í@øM"Q¿åȀl¡êOTHERspp@'¼Ó&Á¾LogParabola?ÑMe±é$O?Ӎ|:
B?çYM'mÙ?Ӎ|:
B?©=xÁ¾Ãù?¿¤nԟ÷?îl(sÖUQ?¿¤nԟ÷?Ò6dKë!2?³äãk%?æäÍÚ
og?³äãk%?¹d'Òí? 2¬$¶˜®?ìÓ{
Z€? 2¬$¶˜®?¿Íh—ÝƉ?ˍÿQÚ=N?ìRíG/?ˍÿQÚ=N?p²Bþol?¬ÓqBí£M?ï|znD?¬ÓqBí£M?ؠϬ-Îx?ºÞ"hŠáy?㯘)éÄ?ºÞ"hŠáy?i7'é»á?†"t0î>?ïŠ[#DÜ1?†"t0î>PSR3FGL J1745.4-0754@2%ƒÀ€æ@%¦<OšÀ9ÿ}úâÀ;׎Ǯ€¿éòzv=Éå@õwæÁk?þ±Ø³iy¿é¢Å¿^ǃ¿Òïò¥¾.é¿×B5Ñëg¿át¨üì'ÓAGNbll@°ü±ë…¸PowerLawTXS 1742-078?ïð¥[2šv?\'p[ãÊ?^µIÑÄÔ?\'p[ãÊ?ï€fíÖÞ?ªxU?nø?æxRH¸†?ªxU?nø?°+?…ÆS7¿È?ŒTÏI°¡i?…ÆS7¿È?ïþ3"Ûæà?ÇÉ2|·Ö?,ÍÏvãE¼?ÇÉ2|·Ö?ïÊ,a~?y°&‹‡ß?zéÿ{^dÌ?y°&‹‡ß?ì¾Ý9Æ9$?ÅIJŸØ€"?º	1Î6ã?ÅIJŸØ€"?ïWJv"&°?ãgjˆº?•±4zaï?ãgjˆº?ïéÛÂÍ´B?bE»tUs?f$=cƐ?bE»tUsAGN3FGL J1745.5+1017@Alú€d>n@3BࡕçÀ9F–µ¹‹À;=4Ä,ë?øtþÂhDã@'žEzÞn?ý©ò!vr¿æњì¢L"¿×•&'¿âDîôàt¿î¶9ÀãWPSRPSR@–ä
"M;PLExpCutoffPSR J1745+1017?¦ä3Þ¹:G?¬¥oUlPÞ?Áøï|?¬¥oUlPÞ?Ã_۟oé¿?Çö;²Oj?ë(	$?Çö;²Oj?Ú²'ò0Œ?µ@àúö?⦷ðgº?µ@àúö?Ô$Z¥	†´?«êLtÙ¸ò?åíÒ­{<¦?«êLtÙ¸ò?xiÙZø;?y´ÈÕ·y?ïÏõ,"®è?y´ÈÕ·y?£Fxa	1?·W0ú"ý?î˘z	ÜM?·W0ú"ý?¹Î²YrÑÈ?ªçÒ¼ÄÏ¥?ìÆ)´Ñ¥Ç?ªçÒ¼ÄÏ¥?«iÐHðCP?':É×.b"?îIbûU~ë?':É×.b"PSR3FGL J1745.6-2859c@vJ r~¿¤¾¿À`2À6	škP°òÀ8f€®I#?Ñ1뷕ûL@ä•Wëy`@'þ Œ=¿ç¥ìù'þu¿åõÁF†Í¿ß%áË·y¿åß äçuÅOTHERspp@£âðå`A‰PowerLaw ?苶ÀØ%?ÐýÛC?ÍÑ$üŸßj?ÐýÛC?ïn{¥+·Ù?©á¨ /?'0‹Whó?©á¨ /?á£Ñ÷Œœ?´z›A<?ܸ\æÆã?´z›A<?ïÌµ'jô?~3t­´?yù¥7zr9?~3t­´?ëz3Èâåñ?Á°Oþgq?Â0Üth:?Á°Oþgq?ëë{fRÅJ?Æ7Y'à´?ÀRf´êÙ?Æ7Y'à´?çø¨×¾Ý?´*ð¤Bj?ЮP'Eâ?´*ð¤Bj?îê€nqÅ?Žéq'!QË?¡WùSK@?Žéq'!QËAGN3FGL J1745.7+3952@Pd™àvp@=	› æÀ:¨KAFò-À;Õ«ïÝs
?áû=ЕÉ@
= åRՐ?ú÷x_7H¿æ£…µOòJ¿ë‰IáZ¿Ú)ҝ'n?Պ`·áêQAGNbll@Ãîxr° ÅPowerLawB2 1743+39C?ïÿ/šPÊ?Uæ'i§?»I &U?Uæ'i§?ïËDgõ?Š8¶+ªæ?z]ðÍeT•?Š8¶+ªæ?ïݼjNŽ?kk3åÀ¥«?q!Êò)m*?kk3åÀ¥«?ïúÆ
àq?9	\"¡?D狾˜õË?9	\"¡?ïý?Fž?5#h…Õ?6ÓÛÇg?5#h…Õ?[þ·?µ•Ìͦü?§ïÐx"?µ•Ìͦü?ï "°¡s?"²E1ïX–?‡û	ˆÏN?"²E1ïX–?ïÏCç?{ é"¿s?x^|ÆzÒG?{ é"¿sAGN3FGL J1746.3-2851c?à ÖdP¿ºh~À5 ÝÀ6‡7`ÆÀ8·*´ßp=@áhy@-5ŠÑTÇ?óËá'LË
?í}Â"¤Å¿Õ¿Ó?,» ¿äè‰÷e&Ë¿êO© ø³…OTHERpwn@¦ëQë…¸LogParabolaPWN G0.13-0.110?JÏèéÒ?l•×L=l?ïùL5E©?l•×L=l?°­¥]½¸l?Är…2?©?íêKTVb?Är…2?©?µÑr¸?¥ÚúÕý*Á?í\%ÜÍ9É?¥ÚúÕý*Á?¶/YM½çÆ?3¶a'?í:ÖHC?3¶a'?|¦¢òív?£onÁ·l?ïƳ̱Û?£onÁ·l?œ[º¨íPy?½<ƒ>
É?ï"*ª×?½<ƒ>
É?¹RO:ø9è?­bÞºh¥?ìÕ¶¼u£?­bÞºh¥?žòʹ˜?ez¿?Å?ïXi'Y£?ez¿?ÅPSR3FGL J1746.8-3240@vO¿Î·‰ÀH?Z³ÖÀ7a<ðKWÀ:0ñ>œ@×Þ§À£Ê@ú§S@™Î@o$¥ü©¿ß}wŸžÁL¿âL2_Æ«¿è™»L
´S¿í<ôàg3kPSRPSR@Ž}ŠüPLExpCutoffLAT PSR J1746-3239?9p<QÉ>¾??"ºµG?ïüÑø¹B_??"ºµG?¨'VCúî?Âl¤Q?î}Š›é™Ñ?Âl¤Q?±ñ2¥_C´?£âë'|?íÁÙ«FY?£âë'|?éMÕٍf?w:Q0†r?ïxµ'znå?w:Q0†r?>Aw
ß,?Dóö"°5â?ïü7ÜÃÃl?Dóö"°5â?ŒȂA?±-Vrô?ï{ñ©6V?±-Vrô?¨u\aJŠÍ?¥j¯Ï¥•?îxª:'£?¥j¯Ï¥•?^µe¹Ø}T?RÒ`2;Š?ïð¥M=0É?RÒ`2;ŠPSR3FGL J1747.1+0139@:õ€`°@.FÓÀ9n‡Êd<ÀÀ;©¿Š¯¿àl
‰_©x@Ò[]@%ù?œx¿å]yfâüÔ¿çv4ËÊÕ¿èŠW+±¿ïþ÷'ò[RAGNbcu@'"Aò×sPowerLawPMN J1746+0141?ï¤äìí?œO}†€i?œËc"ùhP?œO}†€i?ï}¥ì‡ç?¡nDán_þ?KB}æÑ)?¡nDán_þ?í"#2ßü?¡šºÏñ"?·fè Î?¡šºÏñ"?ïÒ§"`CÚ?e>•â^ë?v¬=Ê^³?e>•â^ë?í¢Ó«p?±áÓíÛî±?²éb¦¡?±áÓíÛî±?ì¨&¡÷®o?€¸Õt?º¾ÊðBŒ†?€¸Õt?ë]>ŽÈ?«ãÝ¿Ì?‹ýǸÞ?«ãÝ¿Ì?ìN-Õ6?°àëEfo(?½F'VK‰?°àëEfo(AGN3FGL J1747.2-2958@vt´ ½¿ë@~ D¹À6rA&:ý,À9gåëoO@¾o›Cgß@bqŕ 
@yV-3??ÄéVäEíԿ丄&~Ÿ¿ç*‡ÿs,¿íœ‰8#PSRPSR@–ñòa|ÚPLExpCutoffPSR J1747-2958?RMk•ê«b?X#9t¤šd?ïöÙJVê?X#9t¤šd? üÎ@A?»Â­N­70?îð>"òÀŸ?»Â­N­70?ªˆž³T˜Ã?¡ÙtVè:?îWvóñÄ?¡ÙtVè:?Œ³• '?vÃÞåÉü?ï1©›Dj?vÃÞåÉü?Vِ̌?[éé¯Xã?ïô™ø횫?[éé¯Xã?"DŽP–¢?±…ŽÀÒ·€?ïg™ÃϼÛ?±…ŽÀÒ·€?¬Í)œ÷?¥|ѺÚ?î3-f7?¥|ѺÚ?gÞmPhâ½?b
ÿ:¾Ýî?ïè!'|–?b
ÿ:¾ÝîPSR3FGL J1747.6-4037@uâî_ú;›À˜Ü )€­À8Ü4mÅÖ9À;8>4îõ?ð{"§;™@¶ÇÖÃƔ@•¡ŸÍeN¿¨—ÌöúY¿äìȜÄû¿äâCåe¨"¿ì
tñÅÄPSRPSR@'/"@N¤©PowerLawPSR J1747-4036?鳫eka?Ãü(sÖUQ?É1RjR{š?Ãü(sÖUQ?âî´ûÂ% ?ÉaŒ#±­Y?Ú"–{µ¿?ÉaŒ#±­Y?èt¡ó/b?²Õ·öߗ?Î-x3BwŸ?²Õ·öߗ?åòV§¼?¦Ÿî£ZdZ?ÔS÷°ˆ?¦Ÿî£ZdZ?ÉÑ=£Öp?Åf:
~)?鋰¹W
d?Åf:
~)?¶nøä¶V?¿pǛéÊ?í2 ãi5=?¿pǛéÊ?ÔM{¿F°?¹ú8jՋã?åÙq \¨?¹ú8jՋã?Æ+*ˆI,?¤ÃB,Çʊ?êu5]ý-µ?¤ÃB,ÇʊMIXED3FGL J1748.0-2447@¡v m³¸?û€à»AÀ7VãÉW,À:$GŠLá@ö‡`±ñ@JÁ"àL[?øQO¶ñï¿Í¤‰øóB¿ÞY bvÞ¿äðè géô¿í( 2:OTHERglc@"‡ÈK]ÌLogParabolaTerzan 5?yá+µ*»¶?Ž9¯[õ4¥?ïÌ=¨­à?Ž9¯[õ4¥?ªYV]"Ào?Àìw½?îZjš'³ù?Àìw½?µ^Äaˆ?¦^¶i•E?íT?Ç/ß?¦^¶i•E?µ>ý¶–‹?˜"—KXƒ?íX Ieh~?˜"—KXƒ?‰Í~æto'?'芘tÖl?ï˜Ê«"?'芘tÖl?—eô8'æ?¸ýŸ¨lù?ïDÐ^I-é?¸ýŸ¨lù?ÈSmÕ	v?·}"сê?éë$Š½¢|?·}"сê?"Ö€i?ƒÉÞ¬Xn?ïaO;ã—%?ƒÉÞ¬XnPSR3FGL J1748.0+3405@M¬BŸ·ÀÌ@;.¦ÿ³©æÀ9œV÷]šÀ;É,¨Õv¿À(UR—Òo@†íð]÷@²ÍOÔ¿æ]ìÎ꽿ã—B•¿ç‡@fn'¿ÚI-è½æwAGNfsrq@‹B>À//˜PowerLawMG2 J174803+3403?ï¥yTæÈ]?µÂ'š`ŽÂ?†¡ªÆMèÒ?µÂ'š`ŽÂ?ïÖc™é‡?v†ÙžM{?tòNKÈlt?v†ÙžM{?ï®gÀiÎ6?†²¿\+7?"fÛ튈?†²¿\+7?ïÿÿyÈBú>/ŒC>Ä©åë'>/ŒC?ïô	VLÒ?b•Èv`?WíRÝ'Ló?b•Èv`?î×َYÓ?±€@áíQo?¢'g†è&?±€@áíQo?îþZý£Ò?š^f¶Åç? Vmôè?š^f¶Åç?ïÿæéó=>ó">{=[¤>éÝtw:p>ó">{=[¤AGN3FGL J1748.6+7005@Y!ˆ M@>µ 6×-À7͙ȓ'(À;#Ö~ý6!¿²µ¹¶'à@õ΋"Çs@ƒäŸÒBØ¿àtæu¯¿á'À¦<¯¿àr|Ý~ÔO¿áªÀÐë‹AGNbll@'Ü_ö"PowerLawS4 1749+70?ïÿÅQФ•>óe7}!2ø>ýWÕæºÈ>óe7}!2ø?ïÜì얰u?€ÿÜk,G?q‰‰½–Á~?€ÿÜk,G?ïì"(°­?jrÍu¾Æî?cÝ×3›?jrÍu¾Æî?ïÿþ#B5–>£WDgz‡ý>­Ëí².Ë>£WDgz‡ý?ïÿ or?;r¦iè?à(ôh"?;r¦iè?ï*ôr$­?©"¦/ÇF?š¡q·úÄ?©"¦/ÇF?ïízeæ}'?q®ZL òÃ?b…š[zíä?q®ZL òÃ?ïÿü¼ ý>¾ÍVc¨3>º¹'b>¾ÍVc¨3AGN3FGL J1748.9-2021@÷ŒÕ£5@TRRá#À7éèEÏÀ:"vOèu ?ß²žDÆzñ@‰Õ®óò@aŸØ"¿ãÊc0Q¤¿é~ùÞ1¤¿äy–ÄÓH¿îmÁBá&OTHERglc@'²|PHðPowerLawNGC 6440?ã\—sS›?Í­RáÙí?ÙFÑÿXÊ?Í­RáÙí?듢!†6?Åàs`"?Á±wyç«(?Åàs`"?ã¨A…3—?¶vÍ"†]j?د}Ôõ˜Ñ?¶vÍ"†]j?ëØlkõ,Î?¢Ðö0¬à?ÀžNP+LÆ?¢Ðö0¬à?Ò¦óƒ^³ƒ?ËÇé³:w?欆>P¦>?ËÇé³:w?àÆÒs)?Óã]TfV?ßÖr[ß®?Óã]TfV?á.ª€¥5?ºƒÆžŠo/?Ý¢äªþµ—?ºƒÆžŠo/?ØLUôSN‡?·¾î¿ê%?ãÙÕÖX½?·¾î¿ê%MIXED3FGL J1749.1+4322@Qi # –@=#ì_9K{À9
AðeXIÀ;¬ŽÁÏBÉ¿ùù"Œº8 @úVÆz@ù¬ƒ(¿â‡½m֔™¿åUifK
š¿Þ4
LùǛ¿è¨ú_­AGNbll@LœàuöýPowerLawB3 1747+433?ïûô èq³?8"§ó»*c?@/}+HJc?8"§ó»*c?ïÒ2t"È?‡ª®O¾l?v÷æÈuËñ?‡ª®O¾l?ïÒ¹ì?z¬k|ü?v£x«8ƒ¤?z¬k|ü?ïÿ³<`Œ?l"7SÙ?0×Ù =Ý?l"7SÙ?ï÷ë.À:v?NeÕ>4œ³?P)¢½ªjp?NeÕ>4œ³?ï^‡Êº#?¯!äUìG?ž4/?Á•?¯!äUìG?ïEZŠ û?"I`3W¬?—T®À㮒?"I`3W¬?ïø…ˏ¶?PÄU5嵿?MèҁìUe?PÄU5嵿AGN3FGL J1750.2-3704@v^ FÇeÀ+_ª4œÀ8³¼Àæ½À:éÜF½S³?ï|@Lv@
hhîV	@³Öà¡ëοâÓíçпåjÑfe¿å¸ÜP'`¿ìˆ¡ú'+6OTHERglc@'£ëŸU›=PowerLawNGC 6441?âp2ÂõÞ?̺('<Ðb?ÛÁšzC?̺('<Ðb?×ÞðnÂ?ɡܘ5°*?ä‡ûȞü?ɡܘ5°*?æ´ã´ÅÄñ?²â–yê?Җ8–tv?²â–yê?âaU¼¹Èþ?ª•…á÷np?Û=T†Œn?ª•…á÷np?¶ßYê/Í?·Z†áÀ€·?í$ÂãG–?·Z†áÀ€·?§¯Ùд?¶0òÀÊ?îå䤅?¶0òÀÊ?Ö%[‰á?·ó'0é?äðíRu»?·ó'0é?·¶B"¥e?› š‹NV?í‰7¡¬ã?› š‹NVMIXED3FGL J1751.5+0939@Avf H	"@1¦ý`OÀ7ù¢(´T0À;l5ç?úåÙ¡q@|Z
w¢@5÷Rñj¿Öp†Ҙ¿å=WÏ¿ã Áõ
¿èî>D´AGNbll@…H‰ÞÒLogParabolaOT 081?ï÷•uƒ?QPéJ1?PÔÞà¾ÐÅ?QPéJ1?ï$t«·?´Óª"'Z?›q}°‰6?´Óª"'Z?í0¢ÆO@k?¥èÑÔNŠ?¶zéÍóð&?¥èÑÔNŠ?ï"ÆQ;9›?pfÈø^x?‹k¦âÅl?pfÈø^x?ïà¡lgÝ?qàÖ¿sÙ¦?o^åŽÂÔ?qàÖ¿sÙ¦?íW*ì	Jy?ÂoÎÖ"?µF¨ê¼?ÂoÎÖ"?í"Ži~"?¦9Ֆxf"?¶ëŒ´"e?¦9Ֆxf"?ï0'W)T?‹çoéÚÀ?™û®'?‹çoéÚÀAGN3FGL J1753.5-5010@udvâ—À'ù¶^À9Jûüe@ÌÀ;^&>?Ԁ‹"ò²S@9DM·ÃÑ@(Ððž¿ßk6cƒ ö¿ä뜋ýÈ¿éÊ°¤o¿ïÿÇo.¦AGNbcu@…ŸöݬîáPowerLawPMN J1753-5015?ïà+FÞ>m?hFûÿG?oÔ¹+`{?hFûÿG?ï eoâ?—þ›^½;?‡æœ–I.?—þ›^½;?î,…TÆ´b?›Åˆ¹]?­7ª¶(nÕ?›Åˆ¹]?ïüÚȧ½ã?$ÓƒЄ?9)¼Õ!Nž?$ÓƒЄ?ïÙü2•ÿ[?')…yïâ©?sæšãJ…?')…yïâ©?íVj!z?À"ßm݂?µO¬Í°?À"ßm݂?쟹T†%?¬0;ë•D2?¿ƒ5[ÎÕ?¬0;ë•D2?ïðÑfú?U6±‰Ñ­¹?^]ÉIã‹o?U6±‰Ñ­¹AGN3FGL J1754.1+3212@LÞß¿î—ù@9j´M,ÙÀ7ôkõ oÀ:áNÊϝ?êÆ"Ì¿@Ú¾[?þl>ÙÚ¿Ýö?ý›÷˜¿Ü3
Ú¼¿ÚþE(‰Ñ¿Ýï¯f"AGNbll@šKí'hr°PowerLawRX J1754.1+3212?ïÿ7mª}m?±
|'?OÉ©…Z?±
|'?ïÁ`
©·?"^"~¥?O¸
à€?"^"~¥?ïÎݪ%?{Y3!ô?xõ'	MÁµ?{Y3!ô?ïÿ€+Y>ûD8"´€?ú*\mâ>ûD8"´€?ïþ±:8ú·?!Ѕ³šŒ?$ì]6>ô?!Ѕ³šŒ?îÆy¹ êÔ?²¬ÊÊT×?£˜dq`îÂ?²¬ÊÊT×?ïÍyõ±¿Î?€¡þ£é"?yC @áH?€¡þ£é"?ïÿ_Þ%Ôj?Ò<–½m?<œbŽ?Ò<–½mAGN3FGL J1754.3-6424@t'ñ@ìFÀ2r?©c;À9Îw/†FÀ;­±¨"(?Óº0q.@[¹ïÐ\ú@«r`o¬`¿åø¬˜5&º¿äâƒ3ëXÿ蚓Ð4"ä¿á£¯ƒAGNbll@ŠR$Ý/ PowerLawPMN J1754-6423?ïû×ì‡õz?AJ<zx;F?@ M¢—á?AJ<zx;F?ï¾S$•5²?ƒ‹îÈG?€k6ϳӠ?ƒ‹îÈG?ï¸"ûØ?vöd¤Þö?ø7€h#å?vöd¤Þö?ïÕ͹µ—?YNŸ|ßÝ÷?u#l¬¦?YNŸ|ßÝ÷?ïêv±Ð?wFå¸
?e‰ï8ü°ž?wFå¸
?í!S´pp?»Ï/Lãw?¶õb[(•?»Ï/Lãw?îëp`‡¡—?šKî>W@¾?¡Hù÷…æ'?šKî>W@¾?íûv'_kÿ?›ÀîÂ÷Ô?°$KvNz‡?›ÀîÂ÷ÔAGN3FGL J1756.3+5523@TßÞÛgš@=·™€o&)À:M‡rO©À;áËÜñ?Þ[ǤÍ\ó@o»îƒ*í?ÿ°ð`$ØÒ¿Ø/óÃ[´Ý¿ìn`mŠ?¢A>lTð{¿Ï÷Xš¼ýAGNbll@¨E%`A‰7PowerLaw1RXS J175615.5+552217?ïÿy$.?͆€?/?½Ê	söX?͆€?/?ïÒÓƒn?šñ‡!^?výkOLû?šñ‡!^?ïÍ)]¾Än?zççȸ(n?ykQ¥"?zççȸ(n?ïÔ'aÿ]?`¿!@¬Â?uìO£qª?`¿!@¬Â?ïûفÞ^g?Bĝwñˆ¤?@™÷ž‡+}?Bĝwñˆ¤?îI'"Ø(?³œ6äM?«g×èzKw?³œ6äM?ïŸds¿aÍ?‡ÄàÑ.?ˆ&ã·ðÞ?‡ÄàÑ.?ï//·—uA?©TÔkó0?š	éíë?©TÔkó0AGN3FGL J1756.9+7032@Y?'à°«@=ûßä׆À:Á#å¸VÀ;üˆµENJ¿äó|îí@§†³bîb?ûIÇÚñS¿í8~_\¿æ´
ýÁ§¿ÒÈ ukg¿É…\¾ÐhkAGNbll@Âò¦§ï²PowerLawMS 1757.7+7034?ïÿyK+³ž?	x/KgÏ?Ö¡ñ?	x/KgÏ?ïع•?…¼Ó¾*3
?súx _s?…¼Ó¾*3
?ïéQA³v?]uîú34M?f®¾a'¡Õ?]uîú34M?ïÿ[óEÝZ?¨Â»ã@'?3+?¨Â»ã@'?ïÿPW±A×?ž*#ºt?õ	"
G•?ž*#ºt?îæ7ºßíï?²ç|
ôlý?¡œ"PIS?²ç|
ôlý?ïâŁÜY?làõDƒqH?m:~úžq?làõDƒqH?ï÷#׏bM?R*cÖ¡ß?Q¸Q·õ?R*cÖ¡ßAGN3FGL J1757.1+1533@D–uŸ¿Mˆ@2ߏ`Z³«À:-LBα©À;ŸÙ0ˆ^?ðY— ñ@q•înr@\"Dž?嘖Ät†¿Ø·§.¶){¿Þ™À&Ä¿ïÿÞ&çJ|AGNbcu@¢"oiPowerLaw87GB 175437.6+153548?é·8zÀ?ŗ™"uðó?É#âÿä?ŗ™"uðó?æÀ¾C?ʖƒs't?ÓÒ~ƒyØÅ?ʖƒs't?咘վ&Û?²Pîå¦b€?ÔÚÎTƒ²I?²Pîå¦b€?è'"+Ï?¨·åqÖN?ͻݯPÚ?¨·åqÖN?ã²Þ«Ý?ÐJÍ—ª?ؚB©üEê?ÐJÍ—ª?ØcD–e0?ÍûÛ
Û®Æ?ãÎ]´Í7è?ÍûÛ
Û®Æ?Þã|¹¹ö?¼Ÿ\Úª
¹?àŽuÁ£#?¼Ÿ\Úª
¹?ØXºvˆóY?¹Y--_´›?ãӢĻ†S?¹Y--_´›MIXED3FGL J1757.4+6536@WÑÇ@0q¸@>?ÐàÀ: À
¡©À;þÀ°^×ý?Þ¦mV^u@¥'Ð&Ém@‰ãŸÍh¿é*š=¿ê[Ôþ…½«¿ëW°év?ãP0…•AGNbcu@™È^ƒä%¯PowerLaw7C 1757+6536?dc› ?ɶìà,iÚ?¥Ô9µzÃ?ɶìà,iÚ?ïՕ»¾‡?…[UÁF"‹?u5"ÿL?…[UÁF"‹?ï}_TÞ?ŒLU0B™×?_2/?ŒLU0B™×?ïý©G5?.Îf,S?3'¸ÉH?.Îf,S?ïŶp?I?‰_ˆ?}$ÇÛ¯gY?‰_ˆ?î¿·Í%&?±"°¹R4?¤ƒ,Ñ·q?±"°¹R4?íº/¢k5"?£"MDïWÃ?².'í':]?£"MDïWÃ?ïË5ªJ°—?ƒGvÝêí?ze*¹«t›?ƒGvÝêíAGN3FGL J1759.1-4822@u…|€"ÞÀ'ê"ßÎ1QÀ8þXÒ)- À;S&ìÓÓ?â×Hêæ¤u@×E¼wÀ@^%à9f(¿âö¬…ڿⶰdGŽp¿æ7ƞñƒw¿ærI@¾ÕAGNbcu@'Š¬Ùè>BPowerLawPMN J1758-4820?ïþn €9\?+—X[‹´?)ûÓ`Ù.?+—X[‹´?ïŒRŽ˜3¾?¡³DåòÞ?Œë\g±€p?¡³DåòÞ?ï 
ôVËá?l†kØ?‡ü'ÜŽ—Ð?l†kØ?ïûg'_%?(«DëýX?Bcbòø)?(«DëýX?ïñPâhú?_pVÜÏ?]^;¬»Œ?_pVÜÏ?ìÿ{€~ëm?ÂvÅ'Ö¢}?¸#ýR?ÂvÅ'Ö¢}?îL	Ìî–Ý?È°Š+O€?«?c4†.(?È°Š+O€?ïíØNqcV?Tçœ¢[·?b'±Ï5QÚ?Tçœ¢[·AGN3FGL J1800.5+7827@['~¡Æ@=×ÿ/öhÀ7[M-°<À;>*ðn'…?"­B@EOÐwÒ@È@3KÝ¿ãnÒ]Qâ¿ã¡Â¨0¶+¿áÁ	¾«Ýû¿ä×¼Öú<AGNbll@ƒæLÌÌÌÍPowerLawS5 1803+784?ïÿýä>öYÀŤîS>þpå·‹­>öYÀŤîS?ïÚµ4Í©?ƒ¡®ÇzQ?r¥e{ïŠ?ƒ¡®ÇzQ?ïêÚÅÅã?l
m@h,'?e%:=½Ì'?l
m@h,'?ïÿîžód€>ÔÄt6»¤â>áaF}À¤>ÔÄt6»¤â?ïÿ«ùºãä?rØv±ªÛ?"T¨ñ?rØv±ªÛ?ï2·¨"sr?ªPsè>Ÿ?™©
øAõ¸?ªPsè>Ÿ?ïޕ}ñ?xòq)jâ?pµA˜ä+{?xòq)jâ?ïÿՅ­ÿW>÷è2ß<>õ=HnþÛå>÷è2ß<AGN3FGL J1801.3-2326e@¬ÐDÑ¿ÐB OÅÀ5™þJZ"À9lžéd³@w¹ŸôR@mÁ̾Š?üßÎoU®¿ÑNŠ§ŽNã¿ãoNlt¿å;ÇÁË¿èÙRav½wOTHERSNR@œT»²þÅmLogParabolaW28?ã¡Î
ÜÊ=?Ö^#ª\¾?ؼcêFk…?Ö^#ª\¾?œŠÝ¶vk?¶½²ìӇº?ï©LL¤?¶½²ìӇº?ÔnñžØ´?´
Å÷=+?åȇ0"ú&?´
Å÷=+?•€Gÿl3?ƒ.NàŠ¸?ïSý¿Í¤¨?ƒ.NàŠ¸?Ö$(ÞñgŒ?Ô.¢¢?äí됇L:?Ô.¢¢?z]œ@Ò}ó?'Ó¤Wb½d?ïËDDž:<?'Ó¤Wb½d?à(jǖyv?¼hÏLXô
?߯*pÓ
?¼hÏLXô
?~*˜½Çp?{¾ý'ÊW?ïêϡéI?{¾ý'ÊWMIXED3FGL J1801.5+4403@Q»&ßÓ9Î@;þßnÀ9g½¨l›4À;ÍVØS錿ҐÑ4¡®w@¶6b½m@`M˜¿æ…$J?ÇÊ¿é¡[j'xœ¿ãéUͬW¿ïÿY,t°µAGNfsrq@yøؤTÞPowerLawS4 1800+44?ïÿa&-Â?fIº?Û?°ªP?fIº?ïÐ
‰¡v?"oX²Y"?wùu#"÷?"oX²Y"?;¤Ì(?p|"•u*v?€Ù9Œ¦?p|"•u*v?ïòª6Â?Fj—zûnf?[ßÀó
[F?Fj—zûnf?ïÿ—PÝú?Ƹ…E+Ë?
>²T)R?Ƹ…E+Ë?îª[¸:³?³ª…7'ƒ?¥ZC×	È?³ª…7'ƒ?ïËZŸ']é?»ÕO";?zR°tSo?»ÕO";?ïX's?ñ:?ˆ—ýï ã?"ï±"'<¼?ˆ—ýï ãAGN3FGL J1802.6-3940@v`—ÌÀ ٍ0À7?ep!À:žT~ÝU±?ýaÛQÊÍï@ç%=§*@ñVe'V¿ß·w=ׯ‡¿ån~P›"¿äEdNM¿è ÑxFýYAGNfsrq@'"ᰉ 'LogParabolaPMN J1802-3940?ïøÊfÀÿ9?QcÇÕ°`?LÖd£€^ì?QcÇÕ°`?ïmf‡h?©D,²iü?'S/!â›?©D,²iü?îy¦cùÆø? …xÀÕŠ?¨e™¿‡©}? …xÀÕŠ?ïü<h)ù½?0ßパ?>½«œƒ:?0ßパ?ïÇÜ°ðx?"ŸðÏ2V?|u'œ‰è?"ŸðÏ2V?ëÏ%ï -Õ?Ʉ/ÃÎ;?ÀÃhAH­?Ʉ/ÃÎ;?íóçΕ?£¼Ñ×ù?°`ÇÊg>i?£¼Ñ×ù?ïýܞÑè?6²"h8?7ùŽªæT?6²"h8AGN3FGL J1803.1-2147@ U,î‡Þ?ÊÔ)`T18À7!DҗçéÀ9º[‡SZ@ªu
Iè@¥öy|Ä?ùÍBM­\ð?ïýǯ½®ˆ¿à*Cùb¿àÀfÂ#Gû¿ì¯–kÅSPSRPSR@§Và6âëPLExpCutoffLAT PSR J1803-2149?rx,ы¹?|~¨—iµ?ïÛ¦nǼ?|~¨—iµ?¤ë±¤´G?¼ÜJÈji?î±Då¦ý?¼ÜJÈji?²0ûGþ?¤WªgÆX'?í¼9ಙ?¤WªgÆX'?µKŠÕ_=?›çŒ©Œ¤ë?íVŽ¥}[(?›çŒ©Œ¤ë?[³©ä¸o?c'ëGƒA©?ïò&+@~(?c'ëGƒA©?Ÿ›Sg?°y…
§?ï{%›½X?°y…
§?¡åÇZ	?¢¿QFì?îïñ£'ð?¢¿QFì? L|e™Fi?'ÑÆJ–k?îû89Ϧé?'ÑÆJ–kPSR3FGL J1804.1+0341@>Ô}`}ï@(h³Þ¿=˜À9í´ùqp†À;^èÅP׉¿Ô¹öP©»¦@Ò´WàçŒ@xÀ†‡¿ã' »Ä3C¿å¶ŠE"²û¿ß¿
º9¿æ›kFÜ«AGNfsrq@›/U›=PowerLawTXS 1801+036?ïÿG{i­Ä?ÜMo–Ú›?¸Ûe?ÜMo–Ú›?ïmëwÕ?°Ò–);|r?'B'íy?°Ò–);|r?ïæÃY—²?qs¬[þWƒ?i<¦*téN?qs¬[þWƒ?ïýƒ•eR?¸ŠÀB?3ãVÙ·½ã?¸ŠÀB?ïþùf;Q?"þ³›‡!? nZ‡––W?"þ³›‡!?í&¢e3û?ñ˜ÿ?æ ?¶Êì؅è?ñ˜ÿ?æ ?老° nµ?‡vÌDy?†ÒÓôt¶ª?‡vÌDy?ïí,šå?W6ø5˜Ÿ?bøӀ#X?W6ø5˜ŸAGN3FGL J1805.6-2136e@!5\ ¿Êû@?W¦'À6O«ºbgÀ9yºZÚA*?ü>ÐJZÂ@ì}'%VÒ?ü³~'W0¿Ò"ŸÅÒ=¿áñëjFÆ¿âõѨԠ¿äóEšOTHERSNR@«E8ï5LogParabolaW30?ë©ó]I ?ÉçÖu÷‡?ÁX2ŠÛ‡?ÉçÖu÷‡?ÒrÌM'J?ÎO\¡8è?æƙÙt>Û?ÎO\¡8è?àY]Öc¾/?¶ËŠ)$–¬?ßMDS8ƒ¢?¶ËŠ)$–¬?âJ•a?y×?²n9/ÖÅ:?ÛjÕ=Q?²n9/ÖÅ:?æcø?
ÔK?Î3½²'¯ò?Ó8äWi?Î3½²'¯ò?Àd¹{iáN?Ç=Uº¶d?ëæÑ¡%‡­?Ç=Uº¶d?å÷¶KgBÁ?¶Û·hö?Ô"i1z?¶Û·hö?Ñ5PˆXª?¹'aƒMˆç?çe1W»Ó«?¹'aƒMˆçMIXED3FGL J1805.9+0614@@­çÖyõ@)矾vÉÀ9ìŽÐè»@À;£ŸM7Á7?÷x&º©ß@
'ë¡?Ë¥Öé±4?Û¨¢þiŸM¿ÈÁV8¾.ò¿à«ñ«uÜ¿í-b
çPSRpsr@ofÁ½¥LogParabolaPSR J1805+06?Íי€*mù?П Ç"Û?芟õd'?П Ç"Û?Օm}ºsŒ?Ш…ßlPz?å5IA"Æ:?Ш…ßlPz?ÖþÅ\.ï?¹K¡¥ªê'?äù€Qè‰?¹K¡¥ªê'?ÛêbÁZ?»EJ™Î•?â
óNŸRõ?»EJ™Î•?À,YÃHr=?нDÙl?ëôé-ãq?нDÙl?¸ÜÒÜvÝ?ÄaJŽ'‡?ìäe¤ceð?ÄaJŽ'‡?Á¡-a¸ã?°<K˜?뗴§'ÿÇ?°<K˜?·z¨"òWF?­R¤™{1g?íªïF87?­R¤™{1gPSR3FGL J1806.7+6949@Yñà'Œ7@=-SaÅÀ7÷Þ¡
§#À;Zë´ï`v?ð-3¢Câ-@^!p¾0@ßGŸ¦Îá¿Ý‰V)q,W¿äp¡1'GÝ¿ãOK Î}b¿äë]ö͞¦AGNbll@‹A£S&PowerLaw3C 371?ïÿ›"fF'?­ù°èí?	4rcFš?­ù°èí?ïÒSµðÎp?†_ÛâÞ>â?vÖ$ð;p%?†_ÛâÞ>â?ïÑr"Ù&´?{§AgÉPã?wFµ¢Šî)?{§AgÉPã?ïÄH+½Èù?a#¢‰A?}Ûê4YSy?a#¢‰A?ïÿƒT?
SÀdE?+][(?
SÀdE?î¸;ÕD¸?´Ã=‡ý?¤|H÷7|?´Ã=‡ý?àƒý•?ŠqèâÉK?ŠGåßÒÀ?ŠqèâÉK?ïž¿7&Í?ž"¨<à?L(&n?ž"¨<àAGN3FGL J1807.5-4343@uÓÞ²gÇÀ&9@LzÀ9è6°–5aÀ;xcNƒñ'?ñ&>Þb ‡@î)#øÁ@ö<À$È·?Ñ$Š#¿ÔBÖÿ«œQ¿á~?kOÚ3¿ïÿÞý¦ßROTHERglc@žJ¦L/ƒPowerLawNGC 6541?â9¥<²ZR?ÑfÍAÅOÞ?یµ†›K\?ÑfÍAÅOÞ?Ó]~"âS$?ʺçV)Ç?æQ@¶Ön?ʺçV)Ç?ã±ê–¿Ó?³'$"A½{?؜*ҀYÆ?³'$"A½{?áI4ŠÝOb?®Næ¶æƒ?Ým–êEa<?®Næ¶æƒ?Õ8¤21è?Ðê/nW¡}?åc­ôfç?Ðê/nW¡}?«#o^Ç0?¹èç#~ùõ?îMÉ
·?¹èç#~ùõ?Иt§-A?¼`‰z	(?ç³Å¬iw_?¼`‰z	(?¿ŠÑèk?¤ÿ®^h9Q?ì¥Íâÿó?¤ÿ®^h9QMIXED3FGL J1807.8+6427@W†À
¡©@<ó?ÀàÀ:žQ>ÌÄÀ<èÙrÍ}¿õ"§èö@Dt¤@½_€C1X¿É¯…°꪿à*:ø4Á¿â0@ÔÓÎÁ¿Ø#hÖ¿PAGNbcu@£â°¾
í)PowerLaw7C 1807+6428?ïþ™ç$ðX?6ƒÚF·Y?&a'è²î
?6ƒÚF·Y?ïå4Ý#Ôh?o0ŸHœßD?jË"ÿç‡à?o0ŸHœßD?ï½é}»Ü?"—š×Uh?€… Ï'ð?"—š×Uh?ïÿñ°î=>ÒmÄ&Òi
>ܝèòâ>ÒmÄ&Òi
?ïû´'[Ü?Lˆ[5ß?Cý.Sˆûe?Lˆ[5ß?îþö(¡ðç?³C2 4j? q•n'?³C2 4j?ïUI<×C@?•ïG"÷Åà?•VØh‡4?•ïG"÷Åà?ïÿӎæk? ÍÝ-p'?'ûriî? ÍÝ-p'AGN3FGL J1807.8-5011@uuIàâiÀ,?{@À:¦Ë±DÀ;xût€¿ìäkWšy@înKbª@X+Àx*´¿â%Ÿ¿èðj¿D,¿è ·§exï¿Ë†)žÎ¦…AGNfsrq@'¢'@·€PowerLawPMN J1808-5011?ïýükÝ?Dèʨ»?7(ê"ö?Dèʨ»?ï¹"ô έ?'6"ÂEáì?·Bñà?'6"ÂEáì?ïÃ-zKÅ?{ð™;+?~iBë‹I?{ð™;+?ïÿàšmu>áp`?f=>ïe'2ÞÇî>áp`?f=?ïøu¶w?U»¢v@²Ð?N+ÓÆ+£?U»¢v@²Ð?T?Œ!?³>&†pÁ?¦꽿ñ?³>&†pÁ?ï4à›Ðo]?'Žßw‰¨?™cì‰a°M?'Žßw‰¨?ïýößߒç?,–€­~?0IDGÎÖ?,–€­~AGN3FGL J1808.0+4652@R'³`<Î@:'
4fÀ:ÄIqcÀ;ððÄXŠ¿¶C²"b¼Ÿ@¸Šh#Tï?û¤h_dêe¿ïyATõP?ïi†âðµ¿Û+ý¥Ãڜ¿Ó'ë=Œc·AGNbll@¸ Z^5?}PowerLawRGB J1808+468?ïþÞR[_?JœKÑrª?"ÞÎc*?JœKÑrª?ïг¹°?…gòH*'Û?w¦xX6ý?…gòH*'Û?7F>cú?ƒïè>é
?€Ú.qÆÙ{?ƒïè>é
?ïò½‹!—æ?G•@xÂU1?Z"éãKÒÜ?G•@xÂU1?ïúëãIL?DÑbÈ5uˆ?DSÐ/ÈÕî?DÑbÈ5uˆ?îęZç?®˜žv¬?£¶jVRJ?®˜žv¬?ïžî%É#†?†HÙE}£õ?ˆDvŠG'{?†HÙE}£õ?ï"šëö€?"øù֏& ?Žþ™7Cð?"øù֏& AGN3FGL J1808.5-1952@$ê;¡–¾?£z"`h®<À7֓vié©À9´rcÊ«?ù¥)Gwý@¶ktBG"?ým¤ˆµñ"¿ä»?܎â¿Õܾ²Wց¿çíß¡»§¿é!& þ'ÃOTHERglc@UI7KƨLogParabola2MS-GC01?‹Ê…úÊCØ?¢qüuö–?ïÕèKа?¢qüuö–?Æ?Nñ?ÆÛß!Á¤X?êy°,z~Ä?ÆÛß!Á¤X?Îa'$Ÿ?´,½Å'Nê?èg¶:96Ø?´,½Å'Nê?݇vÈDŽ?±Fg¸©ˆ?á<D›Ý¸û?±Fg¸©ˆ?QT">?T#"‹q?ï÷Uü®3Q?T#"‹q?¤"_œX÷Ï?µÁݖ¯À‰?î·ºõ¸S?µÁݖ¯À‰?»'8¼´ü¡?±.½»Úe?썸èi`l?±.½»Úe?¾¡£"ÃkÐ?¤Km¼›ý!?ì+ˍ‡'†?¤Km¼›ý!PSR3FGL J1809.4+2040@G¬Ì W"ý@2:X@2õ÷À:2@ºˆ'À;¥:Ùâ)?ÜR!ñþpÅ@
·‰Ð£Æï?þ)¡-¿ä¨©¶—¿íõfß捜?ݜ—¡ƒ;¿ÆìàϟKFAGNbll@µà²n—PPowerLawRX J1809.3+2041?ïÿ{&;ÿ?᥶ƒ@Y?ГÉ?᥶ƒ@Y?ï¡j­a¼L?˜üÝQM|??‡¥T–bàþ?˜üÝQM|??ïã°7&)?hºî"Lò…?lOɁ¾ä?hºî"Lò…?ïùbUpÛñ?;ÿµ3
ý?Jv«ӂå?;ÿµ3
ý?ïý?£Ùäb?:¿Dƒ•ú?6ã2U½?:¿Dƒ•ú?î ž÷Zµ?¿:)hüe8?­öŠ^4¶?¿:)hüe8?ェ5{Às?€Þ-S"'?€•r¦ç9"?€Þ-S"'?ïñuuøՔ?^ô"¿?]4Ðw=?^ô"¿AGN3FGL J1809.7+2909@Kás 
Ìã@5F(ÿӊVÀ9
3èdØÈÀ;Lü~¹D?剞C™Õ @×Ú Ÿó?þ}a?5¿Ûéß¿Ø
‡ñ"޿ۊIþYj]¿ÜÜÇÊ7$AGNbll@¥z™=ÙcPowerLawMG2 J180948+2910?ïü"âl5!?5­	Rð|?;Øí«¸TÄ?5­	Rð|?ï¶Ù\õq?Ž""¸h˜™?'z	§ºÁÍ?Ž""¸h˜™?ïàÄøSJ?hÿ̎Aj?oá:ÔÒ~·?hÿ̎Aj?﹢ω{Ð?aA*n•–?—Lá[é?aA*n•–?ïø¿@¿…3?E§V¢ÏOj?MýIïÐv?E§V¢ÏOj?íԒ@+`£?¿Kbvd-?±[müí,è?¿Kbvd-?ï­)`÷f©?…ƒ±»¯?"µ§Â&Uª?…ƒ±»¯?î'Áye$P?"	`ï#?¦ãègõí?"	`ï#AGN3FGL J1809.8-2332@^_±ÁYÀ˜Ÿô|"À5†·¯.VUÀ9Ñ쌅´à@E»ÕX·|@MØÈÙx,@®'oXÓV¿Õ.™1%"5¿à¤Øðz/¿å6KÕQ¼Ç¿ìÆ'ŽmÊPSRPSR@7'l‹C–PLExpCutoffPSR J1809-2332?HÒ3ø2'?Vƒ*çÛM?ïÿ†Ü¹»?Vƒ*çÛM?¡ËS'QÀ?¾b@¼Þ˜&?îïóJñ$?¾b@¼Þ˜&?•xù—ô?–v¬íyå?ïT87::?–v¬íyå?¿®\|†>úy*xͲA?ïÿ¯¼à_k>úy*xͲA?"N9
'§È?Ç+Kàsý?ïþÛ›Â?Ç+Kàsý?zMoô«uQ?›Ò¨!‰?ïËe 7¥U?›Ò¨!‰?€&yPuÑ¥?"6Ä.ºõ×?ï¿fÍG?"6Ä.ºõ×>Ûdì®ÈŒ>à€ûòj‹?ïÿòM²1ã>à€ûòj‹PSR3FGL J1810.1-1910@&">'âÆ?§Q*?ô«œÀ8w~@w¿TÀ9ÄõǗ٦¿ý~™Îr¿:@œˆjÈê@ÅT`)‹j?ïKæ'øm¿êý
!P² ¿à9õÅšç¿äˆc`øh\OTHERspp@»!±hr°!PowerLaw?æ'íÀôc?ÐaHbw÷ç?ÓÏ°$~;?ÐaHbw÷ç?ïTqu§æ¨?ªií×ÏÙH?•qÑLºøø?ªií×ÏÙH?äÇáUšç?´!¿6o?Öàp=TÊ2?´!¿6o?ïÿô <¥<>æ͕µW>׿‹dž	 >æ͕µW?ê>¤éb/?ÄÓ e‹
?ÇmÈZwE?ÄÓ e‹
?ìÑÜï¸<Ð?Ä¡UáÅ?¹q'¬ü?Ä¡UáÅ?éoYÎ
д?°µdëmõò?ÊB˜ÇȽ/?°µdëmõò?ïÿyÅ
X?-Bœ±¼ø?Ça›	Q?-Bœ±¼øAGN3FGL J1810.5+1743@FNÌ W"ý@0Îs`Iì³À8…Í!†b…À;Q€J=:ô?ýû%Þ
¥@––'7þ@ÅN¢zhÒ¿à–X¿äjlÊ9¿æÒS¬âˆ¿îùU=8ŸPSRPSR@"ºškP°òPLExpCutoffPSR J1810+1744?UÄÕŽ?›´°ou¸ý?ìÍ†?›´°ou¸ý?²¡Á‹o7?Å*>0Öü??í«Çέ™ù?Å*>0Öü??Õ²2ëmTu?µLñ®Û)š?å&æŠIUÆ?µLñ®Û)š?¯ìBÆ¿¦?'°'d)è_?î;Ó¯ƒÕ?'°'d)è_?†]²¿ƒ®¹?ˆàëz­ˆ?黎4صõ?ˆàëz­ˆ?—²ÿdŽE?²ÇqÏ=Nò?ïBogÛ >?²ÇqÏ=Nò?³ð)ÝÄÍÂ?ªÃþ42h†?íúÄ+éh?ªÃþ42h†?~¥Àýh"?k½ø(Z9?ï´}ÿ÷?k½ø(Z9PSR3FGL J1810.8+1609@E"©Ÿ¡—@0$™ù;À9Xˊ­mŒÀ;Zˆú%7?ãp+¶s@#»DLÊ@ۇß\òI?ëLøWÙÊ{¿æ/™"9ƒ.¿Ü–æ°N¿æi$nÔ AGNbll@ŸbD"t¼PowerLaw87GB 180835.5+160714?ïüæè×ÅN?7Ö#Ґ¸?8È·©êV?7Ö#Ґ¸?ïYÁÍ??«°^Ä:êÓ?"ß|©~&?«°^Ä:êÓ?ïÊ4ï 	?x>ÎÝUE?zñe{aw£?x>ÎÝUE?ïU‰í²©?tñÃYåU?•NÂGó«?tñÃYåU?ïõàȾ[?U†,Îkè™?T>n™F}µ?U†,Îkè™?ìˆFïcá¸?ÅÔÊI\6Ú?»½È"àò@?ÅÔÊI\6Ú?ïAÁ^7K?"wÐ'<ˆ[?—߇Ô9'?"wÐ'<ˆ[?ììÉCI?¢}ëoþG?¸™µç£ªÏ?¢}ëoþGAGN3FGL J1811.2+0340@?¢æ_E	õ@%8žç·4À9Hê7.jÀ;"nÞ,µ?òî«¢°š@b}¤ñfŠ?û\zßð&?ïâ]¨QÃA?ÃT…µ®oŒ¿Ð}‡0Fªð¿àå…é—†AGNbll@¶&ÐA‰7LPowerLawNVSS J181118+034113?ïyPŒ=B?‹¨Ã—¿±?Õî}"aº?‹¨Ã—¿±?깸"@û?Èú*†™ë,?Åßvü?Èú*†™ë,?î†séu"Å?›èÂHOÕ?§˜Ák:x±?›èÂHOÕ?ìØí&´t¼?˜æÍfìk?¹8–ÉîfŸ?˜æÍfìk?î]ºŽddâ?¦‡•'öWÎ?ª$W¹±ß?¦‡•'öWÎ?äMÕYtv±?Ñ(ȝàr"?×dUMŸ?Ñ(ȝàr"?í*͑¡[?§"ô%E#?·æ©"NÜ%?§"ô%E#?ék'þ¨p?³ð'6?˶Q´^A?³ð'6AGN3FGL J1811.3-1927c@&Cù¡A-È¿Ôñ·€
IÀ8iǾp¸À9¼ÑÇÞPƒ?ìÓNà҂@לã{@áŠÿ¢âî¿çOhË?ç~œóÁ-\¿áú©êIµV¿èpË¡ÖªOTHERspp@±ž [ÀPowerLaw ?ÏÆú:µ?ÊZcMØ?èOqRº?ÊZcMØ?ëY÷Î`Ô4?Å¢ëñ?˜ Æ|¯1?Å¢ëñ?à%ú¾!¹8?µñwǤÔ<?ß´
ƒ¼?µñwǤÔ<?ìç˜?ïw? Åᰐ?¸Ã>êÂÎ? Åᰐ?É®L^†?ÅÓ\"©Àƒ?é"lþ¨^{?ÅÓ\"©Àƒ?ã•ÍK¹?ÑÉ3aù'ž?ÙòÔeiލ?ÑÉ3aù'ž?àÚ|¦CÌ?·l){D?ÞKï³xh?·l){D?æ:Po?»>®¯ˆ÷¾?Óýۋ_!×?»>®¯ˆ÷¾MIXED3FGL J1813.4-1246@1>`ºTû@ˆ•_ùõÀ6¹"ñkéÀ9àЉð@±CÄÐÔï@ÜúE€èž@68õ¿à*¿Þû‡Ë:ü¿å"P3Áoï¿è @*8n¿îE;­nýSPSRPSR@…êŠÀƒoPLExpCutoffLAT PSR J1813-1246?(NNhé–?4vt :Œ¬?ïþ{1è8?4vt :Œ¬?"Ö±Lõ™M?°vÖıï?ïaJuoæ?°vÖıï?¹úrÒÁ•?¦¶#I"Œ1?ìÀ¿ñ¥§Í?¦¶#I"Œ1?6ÂùÙað½?+ü!-Šj?ïý' ­ßø?+ü!-Šj?C4P±?î?Jª\^bíÂ?ïû³ÝM?Jª\^bíÂ?|M"¹Š?©?—/Õe
?ïÇdØi/'?—/Õe
?°¸yiqŠf?¥Ð"·Åo/?íèðÒÄC?¥Ð"·Åo/?QÕÊQÐ¥?	ìj¿VêØ?ïÿ¢¸"ÉÜ?	ìj¿VêØPSR3FGL J1813.6+0614@A»®²@&x¾áQ¿À9JEµì¶wÀ;:,XN?í¡Ô¬rÂÉ@st¤íŠ²?þW@-†?ï©
o6¿ÃWû'e¦V¿ÜPMR÷§J¿áî2|÷CæAGNbll@¬zå¡ÊÀƒPowerLawTXS 1811+062?ïýþҝ5?0¶hª¶éá?0	kä¦?0¶hª¶éá?ïq÷5£r?´]ª
ÛO?'ÁK'µ?´]ª
ÛO?ʌj?‡ž5h­ï?ŒO?u?‡ž5h­ï?ï|/ÿ°?q#ÀùÝ?z
â"%?q#ÀùÝ?ïüы3¶w?:7Õ¼?9s¥&¼öQ?:7Õ¼?ë¨bžŸª?É´â*,#t?Á^u…ùY?É´â*,#t?ïLñ|ÑÚ?'ƒûÉ>Â?–aÐ]-¶$?'ƒûÉ>Â?îŠ*æS\?"MêÚÙô¶?§]_šÊF?"MêÚÙô¶AGN3FGL J1813.6+3143@MU§€)Ú@5Y‰?¯BxÀ95†S€À;…¿üñý?õÐq‡¿@ð`±¿Ÿ?ú­ròe㊿ÕWøÿi¿ß¯ˆ:Ãí¢¿ç(´Ù¿àÇæ|²iZAGNbll@Œ¹Ò½<6LogParabolaB2 1811+31?ïiÚðì?¬3A¬åÕ?'Ü|iÉL"?¬3A¬åÕ?íG$<90?¼øÁ®qÔ?µÄތ)ÿ?¼øÁ®qÔ?í÷"…ÈÆ? ¿-9åx?°C_ƒÑ¹Ï? ¿-9åx?ëº*²Ÿé¯? 2ÙTÇ6ô?ÁU5€YF? 2ÙTÇ6ô?í#Áµ?¸ÆKhßž?¶çAñ{¨¤?¸ÆKhßž?áÀ¦K?ÐXM¸´UÌ?Üгi×é?ÐXM¸´UÌ?éâ·U+?²Ýٌê,Ü?Èu"«£T?²Ýٌê,Ü?Ý:Ÿ£žÖ?ÀAp(Ã(ð?áb°.0"ó?ÀAp(Ã(ðMIXED3FGL J1816.5+4512@R6¢Àh¡@8Àæ_E	õÀ9"¤úö«ÃÀ;µ(Ùº?úDن@p…qœ@äe½Ÿ¿×-ó´±è¿à0Pÿ³0¿ãꯋ?Ü¿ìÊ9­~[ƒPSRPSR@ŒqY³Ð|…PLExpCutoffPSR J1816+4510?°
?‡Êý#?²±ë¸ßÕÊ?íþ¸Ϧœ?²±ë¸ßÕÊ?½E1 ×?Çr²=ï·?ì]×\ÙÛå?Çr²=ï·?Ù99®2¿?µYj[fή?ãcc(栀?µYj[fή?Âào›29Ó?œ¿-G£è?ëGä3q‹?œ¿-G£è?s~­±[ß?€»‹ƒ™a?ïÙÇwBq?€»‹ƒ™a?«-ÿYÌV?Àc\2}M*?îM 
G½À?Àc\2}M*?³ÕœÖÅ1?¢iáË*™?í…Le^S?¢iáË*™?'šê2«|?t\èÊjƒ?ïwÛ(…/T?t\èÊjƒPSR3FGL J1816.9-4944@u† fèÀ.X­~«À9ülhÞæ«À;Ë?'‡]?ö
´ynÖÍ@·Ýª»ú?í{xg«ñò?ïGãmðjÙ¿Û0!œõ¿ååÏA"•–¿ïþ'B)'˜AGNbcu@"âoŸ¾wLogParabolaPMN J1816-4943?æ#8SÙpõ?ÎÁÅ좙â?Ó¹XM?ÎÁÅ좙â?ë×bz‹Ú?ÄfcX·H£?À¢w†Й?ÄfcX·H£?àŸ´ìw8?·|":Õxt?ÞÀ–'õ?·|":Õxt?éK_æÕ?°Jb=<Æ?Ê҃ýÈd«?°Jb=<Æ?æ»YҞ?Ëiªüöê?҉ÑLZÃè?Ëiªüöê?Þ±O~ÿv?ÑÍÊT2Ã]?àù§X@€E?ÑÍÊT2Ã]?῀ل@A?·µ4œc?܀þL÷~?·µ4œc?×äš­a^?ÀÙKq~¯?ä
²ó)OQ?ÀÙKq~¯MIXED3FGL J1817.2-1739@*Ç$ß³Y^¿æ-£€Š#À8@5¾þ­ðÀ9î'Iü?óEêmFª^@ŸŸšm@+/ŸÕÈÊ?å´õ«gâ¿æ˜"üS£¿á8½`É¿èš´¡²ÂµOTHERspp@¦¾¿|í'hPowerLaw?ÜB0iÝÇÏ?Ñ­à2°+?áÞçË?Ñ­à2°+?ꦯ´e?ǹ»/
;?ÅeA‹™.m?ǹ»/
;?á;€ÿ;Ve?¶Çk§?݈þ‰S7?¶Çk§?ìë¿÷À°?˜º²‰x»Þ?¸¢î9?˜º²‰x»Þ?Ó¸Oɺ?Ð"K™?æ#Ø{›p£?Ð"K™?áû›v¬?ÑóG÷K· ?ÜüÉÚ¨?ÑóG÷K· ?Ûs7«Ï~?¼ÏÌË9µ?âFd*yÁ?¼ÏÌË9µ?èIpr•?²k¯?2H?ÏÒÚ>5«ð?²k¯?2HMIXED3FGL J1818.6+0903@B¯¸Ÿï0@&¿ãAƒXÀ8¾Š¯ñʳÀ;0žHUh¿íû¨V@wEöÚ<w@ð6îÍ©¿ã69Àk¡¿ãÆX¶È¿ç.«'5>s¿ã+h¸óswAGNfsrq@Œ3~|âPowerLawMG1 J181841+0903?ïþzwüw?#Ԑý`?(X.غÃ?#Ԑý`?ï:~^³G?ªmg|/S?Œ±`^Z<?ªmg|/S?ï¨à͛åà?ƒp±mö¨"?…Ç̎·³ù?ƒp±mö¨"?ïÿDòUûé?É¾Õ¬?a®"›?É¾Õ¬?ïôÞ­ä™?[¬§êõiÀ?VB¤.ŽÙÛ?[¬§êõiÀ?íÇo>ž™?¿,ý퉹Z?±Ç$"S==?¿,ý퉹Z?ï8MÁÔÌ ?'ÞÎ*L…?˜öGÍýÿ?'ÞÎ*L…?ïôï/)b?RuW"'>?V!¡˜õ?RuW"'>AGN3FGL J1818.7-1528@.ù"!bPW?ƒþèÀ(½¤À7söLø×À9 Š(Ž"@þê<F'@Ipû@?ýr9΂Úe¿ÃQ²º§Ü(¿æ>ÕÈôÐø¿è¼*2	h¿êÖ#ú±OTHERspp@'­>«6zLogParabola@?×9èþu€$?Ï1€d®G?äc€Å?î?Ï1€d®G?Ã,ðÓÆ?Ç"Dt4k~?ë 4ÿCË?Ç"Dt4k~?ÓÚÞB ?³ž{1¢Û?æñ^°?³ž{1¢Û?Üw¶ƒ<és?³òy ¶Œ?áÄ$¾a‹G?³òy ¶Œ?Ù¾4n¼t?Ðñéne…¸?ã åÈò!Æ?Ðñéne…¸?°>ÊSl?¾ýó¶E¡Ë?íü˜&§ßƒ?¾ýó¶E¡Ë?à=-eœp?¿6›²´¯?ßÅ¥4Ç!?¿6›²´¯?ɛ·åù³O?µ"Ú"Ã?陁",?µ"Ú"ÃMIXED3FGL J1819.1+2134@H'ŸÀ$GÞ@0}>ö?À9å(¡ù¤À;Š¦8
‡¿¼KŠÔ&¿@'ÈVñSj@¨_Û÷¿á֟ÞÏ{¿ãè½YDóX¿äv'6+"µ¿²^B¸XÃÞAGNbcu@šð–8†YKPowerLawMG2 J181902+2132?îï"oä?ƵZ·¨ðœ?¡¹.bö?ƵZ·¨ðœ?ï¤|·6?›>fŒÞâ?†ú?'±j‰?›>fŒÞâ?ïsÓÉ7¹?'‰Öè`z?'EŒrÏ?'‰Öè`z?ïüÀ‡V?(¦Ã6j²?9ûÅÆøKä?(¦Ã6j²?ïÌkÆwž?"ĨùÏ]x?yÊ°ó"?"ĨùÏ]x?î´°‰Mù?­\%rdÓ=?¤´÷pžÕl?­\%rdÓ=?íó³â'?©
P[¥&Ç?°bg/¥dG?©
P[¥&Ç?ïÕ¯S.)?pœ6iäï/?u(V~C??pœ6iäï/AGN3FGL J1819.1+4259@Q©'ŸÐ€@7¸ß_vˆÀ:<³Þ¿=˜À;ΌQ²z;¿Öô&žáhK@¥²YY·@߃]ÿålòÊÀᐿî'ÜDÓ³`?ÚuYÂØÆð¿éü½ðˆ`.AGNbcu@ŠÅ
žƒä&PowerLawNVSS J181927+425800?ïþxxY$?#Lw ñÓí?(x|"yo?#Lw ñÓí?ïՕ –¬?"JÿÓ??u5o½˜øm?"JÿÓ??ïÇtéñ?vËTޛڦ?|Eÿpêu?vËTޛڦ?ïü@ý:Á?3ÝlÕù-,?=øpX©š?3ÝlÕù-,?ïþBÍ9s?/<Íè& ?+ÞŒkî€?/<Íè& ?î֋½b÷q?°¿†ÄÒ?¢—D&`ìô?°¿†ÄÒ?ïƒtL¿1•?d-ÌÆË?"ìڂnº?d-ÌÆË?ïð&s‡6@?c¡ý`Qp(?_³+LðV?c¡ý`Qp(AGN3FGL J1820.3+3625@Oõð ¬ @5'â_ܪÀ:m&!Ò¸ŸÀ;ÓùrGE¿ã>ªCF7@x¹ÖÐܧ?ümá?¥¿æcÝ	ñ_¿æ¶[[	f¿Ö'÷6‹_ù?¾d´AˆAGNbcu@· ¨õ\PowerLawNVSS J182021+362343?ïÿoñChy?
oîGœ?Ùe"9A?
oîGœ?ïÖH/)õX?}PP÷%¨<?tÛèJ	"?}PP÷%¨<?ïäg"ãBõ?cò¯ÈJ«!?k˜zÚċ¦?cò¯ÈJ«!?ïÿ gF¾´>û5\Š"?æ)÷@>û5\Š"?ïþþ2us?ŽGyo]? Ü8]?ŽGyo]?ï8ˆ¡hŠ?«©A»é´?Ÿ¸î튼Å?«©A»é´?ïËz¥žÇ?yBïÜKæÍ?zp£øË?yBïÜKæÍ?ïúÔŸ?GRÆh³x?D¬F~ªì–?GRÆh³xAGN3FGL J1822.1-7051@t:gÿyÈÀ7.L`*ãÀ9õågÎEÀ;«¸ÕŸf?ÆG^™‹@EôZƒG@Ÿ¦ e¦"¿çµ¾t´ È¿éJÐeUË¿æ	c3´–¿ïÿƒ£žÃAGNbcu@~:}ÔA5PowerLawPMN J1823-7056?ïòR\2?°*2p¥?‹ÃkoÒ°B?°*2p¥?îñJOPí{?¢alRIà? ë[
AV?¢alRIà?íûÄ3B™û?› Å»i*Å?°!Þhñ¦?› Å»i*Å?íHþ³z§?˜‡ÓFÚ%?µ¸ˆCÅ?˜‡ÓFÚ%?썎?"¡æó~7?ŠÄç
0c?"¡æó~7?áfی‹Ç§?ÒÛè~Y!Y?Ý2Hæèp±?ÒÛè~Y!Y?íx`äÇ?¦ÄÕ/èh?·¿>°§Ä?¦ÄÕ/èh?Öl$…4L?¹Äð)ÖÇ?äýIí½eÚ?¹Äð)ÖÇMIXED3FGL J1823.4+6857@XÌm_êKc@;­5@S­&À9`žc,öÀ;Æ\>'ãÀ^ÙH0Em@¬àÑ;œc@DI€§…@¿ä™Wž'>ñ¿åFfËÞ\º¿ÞZ'qf¨3¿ë!Hï ùAGNbll@'õ4êJŒPowerLaw7C 1823+6856?ïã'DØ?n@€ÂíÚ?l}»'ïïM?n@€ÂíÚ?ïܛA9†4?ƒÁ»ƒ±Ö?q²_R¾ÆQ?ƒÁ»ƒ±Ö?ïQÓËæë?ŽQ÷ºgT?•ßEˆ:ð™?ŽQ÷ºgT?ïÿývbÝÆ>¶3ÿ>2I9>´KT‹¯é>¶3ÿ>2I9?ïcðH¯?"ó;,™¡?"öÿjÃ?"ó;,™¡?îÿ Žj?±=Kö.¸(? ÝöCR`?±=Kö.¸(?í;…õLô?¦m_î–åÏ?¶'›Ïy±d?¦m_î–åÏ?ïÿq<ƒ>?ށÇÖ?ØoùáJ!?ށÇÖAGN3FGL J1823.6-3453@vjá€M˜9À#Þ\ÀjTÀ8ƒè!¼é*À:ۚânõ?ì÷lN˜ûu@àóÇ™?ûùI þ?•jy³íz¿Óoò:îé¿Ó¾Òƒp'¿Ý«xÊþ&ÈAGNbcu@¯Ö@Þ҈ÎPowerLawNVSS J182338-345412?ïÝné["?w¾ÀÎÉr–?q}ÈjUöå?w¾ÀÎÉr–?îޘ–†·?«°R8t>?¢vš(DI?«°R8t>?ïe›T¨K?Ž‡¬ø•)R?"L•º''?Ž‡¬ø•)R?îµÖ%ªÎ?'˝b|?¤¯œÉl?'˝b|?ïpƒÊ
¶Î?mç±(8?'ñX5?mç±(8?åôJ]Ø^?ʓÕ¯ä#?ÔkDOBç?ʓÕ¯ä#?îÂ%2$т?™üÑùçŸý?£Ý¬àFœà?™üÑùçŸý?ê§F¼±?¥A«iuŸ?Åbåí;‹?¥A«iuŸAGN3FGL J1823.7-3019@'œÿT´bÀŸ!€nÅÀ8ÜMÂ*²[À;&œKû?ì)¯‹žY@
þ{uí@yoÿl\J¿Ò>ÕÁp«Â¿áôôç0¿ä8úC8Ë	¿ê'ÖwŠ?PSRPSR@˜q`
qvPowerLawPSR J1823-3021A?í±Z"Õ?µœ}˜&êà?·bu0§¿V?µœ}˜&êà?èý.Î?ÍHùõ`%?ÌGëÀÇ ?ÍHùõ`%?íV˜Ï*†?¥f'ûÛI?·
K8<ÑO?¥f'ûÛI?鄖-10?¢ìä|‰?Éí§K;›??¢ìä|‰?ß}ÓB»D?Ì×£¯5üÖ?àA1^¢^?Ì×£¯5üÖ?×	>Ïë݁?ÒûôՐô?ä{`˜
@?ÒûôՐô?ä3nGcõQ?»ÅȔ·e:?י#q8_?»ÅȔ·e:?ÓR(@ç?¬ËäK±á?æ}øÖëߍ?¬ËäK±áMIXED3FGL J1824.0+1017@CŒß€-·É@%g‹_D36À9®TDZ±À;a~B%>~?óîÔâø@²¦Ú?ÿ×>€C\K¿·O£°•Ä¿Û»vžAôí¿×agnN<N¿îQo3òÿDPSRpsr@¥E›~ÿ—PowerLawPSR J1824+10?Æh
'‡P¹?Ájá/ë?êeý_^+Ò?Ájá/ë?ଠÈÀ?Íò™ºü–?ާʾn~ý?Íò™ºü–?àƧ /ò?µž©¡?#ƒ?Þr±Æ¿ ?µž©¡?#ƒ?æéáãŠS?¨Û%
hž+?Ò,<8ëXÿ?¨Û%
hž+?£ò¨L}æ?¢Óäà!»?îÀÕ›8"?¢Óäà!»?ËÅq™u\x?ÉòÙ4þÔ ?飙¢¨â?ÉòÙ4þÔ ?ÈÇø':á?³ê{ož.»?éÎ9ßqH?³ê{ož.»?×LŽ·¾H?»'Çڟž@?äYô¸¤ Ü?»'Çڟž@MIXED3FGL J1824.2+5649@UnGßþù@:ÀÁ%ÐÀ8Iò×sÀ;‰ùÖñý?趃Q¹±@%͙ü@@®?Æ ¿ääÛ3a=¿åŸÿ«±¿çQIß/¶¿é‡pu«ÒAGNbll@T9ÀëíúPowerLaw4C +56.27?ïþŸÍ\·?!$ שçþ?&-uý—?!$ שçþ?ïÏèiF¦¿?ˆ]ïØ9é?xËS
¸·?ˆ]ïØ9é?ïÐjB,äÿ?rTê¢$Ÿs?wÊÞöœR?rTê¢$Ÿs?ïóeòfÿ?@ð¯Þˆ¾?Y4Ä}À?@ð¯Þˆ¾?ïý­Z'­?1x˜¬õàf?2—ܺª¨Y?1x˜¬õàf?îéåý¨ëO?²"
…®Äé?¡a (àç?²"
…®Äé?ǙK?†ôCŠù€¥?‡þÖQ‰I:?†ôCŠù€¥?ïÌZÐA\¨?qJÝu›Ë?yҗñ/£ù?qJÝu›ËAGN3FGL J1824.4+4310@QÇß 'á@6ÙÙb¶®À:Íú8?ânÀ;øIlÊ.?ӕˆª€i@
"mã]\ý?û˜ÔÀ6;{¿ïÐwwclj?ïëé‹Û|#¿Ü P¤Õ"N¿×Œ0Nk6ÊAGNbcu@¹Îž¸Që…PowerLaw1RXS J182418.7+430954?ïþÄ
}Ô¹? B|ìâa&?#¿[þïø? B|ìâa&?ï°Mˆ§Œ?‰¨ZÝË5?ƒìã+d,?‰¨ZÝË5?ï½Ì°·V?€…ÖB¿?€ŒÓÇ?€…ÖB¿?ïvjã×3?z`
±{¹è?'2£…ž¦?z`
±{¹è?ïúçoîØï?A¡zÛ/½?Db?èͳ?A¡zÛ/½?íëú¤^?¾'|=Æ?·8 /é"?¾'|=Æ?ïr;Õ áÕ?³.Sø?'¸…UZ?³.Sø?ëW–¾·¥?²UEtía?¡¥!kÏ?²UEtíaAGN3FGL J1824.5-1351e@1'A@<02¿Ý`às%oÀ6Œn~bÜnÀ9*Š§ŽNã?öWvšÙ@'
äµvÅ?ËÝJ9pJQ¿ØèPKqîZ?é«\ÚÌiÐ?à(‰¡~ëC¿Â²_8IÈOTHERPWN@Ú¾ÎffffLogParabolaHESS J1825-137?¹[êS!?È<èFX‡‰?ìÜt'ˆÛÜ?È<èFX‡‰?摍 lš?Ò	Uwx)?ÒÜå¾á&Ì?Ò	Uwx)?â>uJý Ê?µÁ¤e$œí?ۃj¾l?µÁ¤e$œí?ëÛ·3»÷Æ?°žyR¿O?À'#1 è?°žyR¿O?ÊI/‰Z‡5?ÉÚgș¿ã?ém´©^3?ÉÚgș¿ã?Ý~x.B'(?Ôé`ðõdà?á@ÃèÞ·l?Ôé`ðõdà?çõünم ?³íE©‡—?Ð"LõÁ?³íE©‡—?ë[½ÝÞv?¹W+O@o?'ôˆ†*?¹W+O@oMIXED3FGL J1824.6-2451@DHÿÎ+òÀa'ßÂó°À8E3å	ÚtÀ:Û5ƒo‹©?ü×È j® @ ½Ã@@"4"¿Ù­`Ç|<"¿ãs§ªyª¿åýÎl+™®¿îb!%û£`PSRPSR@‹ù~Åm\ûPLExpCutoffPSR J1824-2452A?‰WřÊÂ?Ü"‡H?é€Gõ?Ü"‡H?¨ä;|£´?ˆݘ»¼ô?îq¼HK?ˆݘ»¼ô?Öþ,§d¿?µfµIÄd?ä€é¬Mó ?µfµIÄd?°®Ý¹AS?'ÏdbÈO¤?íê$HߗÖ?'ÏdbÈO¤?Cvøqßµ?JΆvFØ?ïû"BH?JΆvFØ?':ÜÞz»?º7êC*Ö?ïn/é&ʚ?º7êC*Ö?¥ªM'ƣ?œš_
~>?î¥[#'+f?œš_
~>?€w̚*?lòÃAÔ¦?ï¾#ñS?lòÃAÔ¦PSR3FGL J1825.2-5230@udS_ôöÀ1w?› 'À8Óû|ÀÙÀ;Z*¤ï82?õŸ©X~qJ@óE$Í>ã?þTK'ôà¿Ñô]%†2›¿ä]rÍä
<¿æ˜ëK#¿ä±Çã%AGNbcu@†U'œàu÷LogParabolaPKS 1821-525?ïûé#´Sô?@݉Ÿ?6?@[qŽXƒ'?@݉Ÿ?6?ïªÓñ.Uÿ?–È°XXùÅ?…K´j€Q?–È°XXùÅ?ï±aêß:?'¨Í¨ºªÔ?œ‰ÓÇ˂¶?'¨Í¨ºªÔ?ïéx֚DÔ?M«Ò2b4?f‡)J>L?M«Ò2b4?ïøe^uùy?RsA‹eÇ?Nj‡#W%?RsA‹eÇ?í"ƉàM?Áّðò‹?³a˸ÂØ?Áّðò‹?îÈî"=b?˜¾hFü™?£qÍß·Ú?˜¾hFü™?ïĐìT…?pÏ1®à?}·‰È®îŠ?pÏ1®àAGN3FGL J1826.1-1256@2Žwß4®]¿ØJä@m»À5š'3K†çÀ9y[ñ˜^@	o_F6›@™åX3ô@ÃTUýŽ¿ÕmW=mc¿âš !¯¨¿æ嵕3êy¿îj+.¤O¢PSRPSR@ŽÜ·`¿]yPLExpCutoffLAT PSR J1826-1256?-Öí%³m?&Ôð9ÏnI?ïþ"'
»?&Ôð9ÏnI?Ï‹¬34?°'ÇÉ4H?ïy‡٘&?°'ÇÉ4H?‰]K&óH‡?Œ¢dC¥?Ó-9?Œ¢dC¥?6Fƒûn¯|?),§øßÕ?ïý7/¹x?),§øßÕ?/v9o¾ô$?!æ±Êü'‹?ïþœ0ͨ?!æ±Êü'‹?lÊea';?ˆTžã'|˜?ïã5št=?ˆTžã'|˜?y0Kȏ.?sIü#'¶0?ï͟h™$1?sIü#'¶0?K2
üøu?¶oêÄd?ïÿe¦MC?¶oêÄdPSR3FGL J1826.2-1450@0â³ÀŒLª¿ô³b ‰!ýÀ5þl3/uÀ9ÂQvYS?úȉ+bYf@º¯¾Ê@å¿ÉY$ß¿ãº/§î¿æâƒb ‰"¿éÑQa£Ê¿éh'žùTëOTHERHMB@q…@áqŸ€LogParabolaLS 5039?³Kü¶R¨?¾F?Ö1?햀i5½k?¾F?Ö1?§¦«h/1?»Y d›Ø[?…;¾?»Y d›Ø[?ØTŸ-q2?´Ùf	r?ãÕ°iGtç?´Ùf	r?Åè*"[ʵ?«tçÕß?ê…õZé
S?«tçÕß?–SVÆ®?¤CِC?ïMeIÁü ?¤CِC?o3çj?¯%yˆÃbµ?ï'A‹'?¯%yˆÃbµ?ÕÅ39ØÎ?¶ãcq¢+?åfcÿ?¶ãcq¢+?›)6¿‹™ò?"OË@Z'?ï&¶IõäÁ?"OË@Z'PSR3FGL J1828.4-1121@47	 :2+¿ÁËTŸþÀ7×ñ
õ´À9×!éBN?ö*mþ¶)@P
º?<@kÛ±í¿Ç´5§+Óm¿çN'D~ˆ¿ì½­?h˛¿ïÿkOÚ2çOTHERspp@ƒô+ÓÃaLogParabola
?åÕÈÁFÔ?Ò9ȾuF(?ÕÆTn}rX?Ò9ȾuF(?è2±'Õ±ù?Ìÿz)6?Ï5;`©8?Ìÿz)6?Üz÷êª$Ï?´P&<ûj?á"
ªí™?´P&<ûj?ê
˜ÿë³?£z©ó¼¢I?ÇɜQ3¤?£z©ó¼¢I?虲`ºÕÔ?Éó23¦B?͙6}¨¯?Éó23¦B?Øt.˜Nú?ЋŌwÙ<?ãÅè³÷؃?ЋŌwÙ<?ãmd?½m¸ë'H?ÙÉ%6ßÿÉ?½m¸ë'H?یîEBV?·ãhá_?â9ˆÝ^ÀU?·ãhá_MIXED3FGL J1828.9-2417@!Ž¡à×ÀÚ{þÀ92t]ŸîGÀ;r«G¿ñàÝ"Zrè@U<Kv?ÿÃÁá6fD¿ë9Ó>'5¿ÑÆ3îˆÎ¿áŸ‰¤X
¿Ø{Úp=CœAGNbcu@°
²£S&PowerLaw1RXS J182853.8-241746?ïî6?"O?`}Zûw{?aÉÀ˜«ñØ?`}Zûw{?ï41…‰j?­@4ÉÇp?™yÏGýúÕ?­@4ÉÇp?ï‰t…/v³?…™¿µý‹?¢ÞÅP_G?…™¿µý‹?ïÿŠçF˜?¢ðóZ°Â?
F(‹rÂÑ?¢ðóZ°Â?ïÂp)!¦2?|q_vÜ¢ý?~ÇëVo·??|q_vÜ¢ý?ìd$Â#á?Æ"ë)â°?¼ÞÙîãö?Æ"ë)â°?îè{ƒGâ\?˜srï;?¡xGÌ]ÁE?˜srï;?ïøq~¦ä?HdRhçp?N:ÿˆQÄ?HdRhçpAGN3FGL J1829.4+5402@T·W?íUÙ@8Ê	?Câ®À9§0IAÀ;¶½ã$þ¿ÚFØRM;@´
Öó—<?þè`·Ð¼¿àjï7/í¿à—j,Õ²¿àº-°3ÜH¿ÍÁ:Áa›AGNbll@¤N²£S&PowerLaw1RXS J182925.7+540255?ïÿ-î¶è›?päƒq?B&ô_Rä?päƒq?ï×ÆêA?"'Y'ì¡ì?tùiD³?"'Y'ì¡ì?ïçLŽèªh?fàº»3e?h³qHÏø?fàº»3e?ïþ)×ruÇ?›5ñ-›?-b†a"ï?›5ñ-›?ïý…OŠñ?0 <Þ0Â?3×èÐ&×?0 <Þ0Â?ïϖfð`?«'¯e>æH?F
/²Wþ?«'¯e>æH?ï¢wÃIÛ?†îԂ¥k?‡b7Øä?†îԂ¥k?ïçh¢q?b¯µ‡-RÁ?h—æJã"?b¯µ‡-RÁAGN3FGL J1829.6+4844@SNü_Ìï1@7|5_]]©À8®¥|%ëLÀ;™—û3èe?æH¢R(@eàÚv@뮟e5¿ãoÉ´i~Ÿ¿årcÎö6—¿æ 4=tU¿é¨e¾´AGNssrq@"*TɅðoPowerLaw3C 380?ïþ¢÷U?&¿ñ3þS¤?/~Ëf¥?&¿ñ3þS¤?ïÃ~E4Š?"ŠY¼ˆ&Ã?~@ø×æ[?"ŠY¼ˆ&Ã?ïÓDUøãŠ?ia¼ó»?v]Õ<ç?ia¼ó»??V­?nÂ?¯à.\?°&±^?nÂ?¯à.\?ïûèÚÁÏ?Bðà%É?Cø\ÊLK»?Bðà%É?î/jº»?µ–g2"°«?­	TZ¨Ë™?µ–g2"°«?ïU\gMÛÅ?ÝÓu×tP?•TseOo?ÝÓu×tP?ìI…–=«?¤Fù1ÜP`?»³ÓNª?¤Fù1ÜP`AGN3FGL J1829.7-1304@2ÚB×P´¿ó|ÔÂ^À8d"_õIÀ:&²ò0?óYœƒÙ¾Î@̼¥BÉ@öc«Kž¿ÓR|¤–LÞ¿Ù¤Ò}ö¿çw,ò§Qé¿æ‹(³OTHERspp@§'…¼£nPowerLaw?ѳo®Žž?ÍË2@̓4?çr¦H(¸±?ÍË2@̓4?â½'ÏcW?ÏËTey?څ°a9ßR?ÏËTey?á~§×ÂA?·!\Œ)
ê?Ýü°P{?·!\Œ)
ê?èâ;'sHˆ?¥÷Þ[`;?Ìwö2Ýß?¥÷Þ[`;?«GÐצù?¶Ð»µ´hŽ?îK'ò…p?¶Ð»µ´hŽ?Śd;¢ ?ÆÓ\à?ê™fÿqx?ÆÓ\à?ܼ¬iç
¢?º_‰N·?á¡©Ëz¯?º_‰N·?Öi¬KÍÞÆ?µ©°Ùן?äË)ڝ?µ©°ÙןMIXED3FGL J1829.8+1328@EQÅÑqw@%ŸàAׁÀ9øŽ½À;e×F£R€¿Ë×¹"Sš@
]|DÊ	y?ýîÞÀX¿è|ãN¦?Å"›-¿äž,÷b€0¿Ü£³Úž­¼AGNbll@±çº=p£×PowerLawMG1 J183001+1323?ïùõWS?PQv
ÀyÈ?H+ïb!߶?PQv
ÀyÈ?ï™\‹#è›?œÿ‰æÝ¿ð?‰¨Ý)GiO?œÿ‰æÝ¿ð?ï©
-B¶ç?€‰$z/?…¼´«âª+?€‰$z/?ïó-m»36?Iù<0në8?Y¥$RŸÓþ?Iù<0në8?ïËùóÌjý?€½Sњ@?z6§9F?€½Sњ@?í±+AÞWö?¿Q+^ʑ?²v¥ñ{3Ñ?¿Q+^ʑ?ï–ù<}›?˜qðza°?Ÿ
 ё«?˜qðza°?ïP
¤Xdp?;¨Í"?•þK{Ò©ô?;¨Í"AGN3FGL J1830.0-4439@uâ!€M˜9À.Oó v,­À8ÌÌ#Y¡\À;q¦½n‹?öê—é@Jô@c‰ô5–@&þûɧ¿áun°Ñˆ¿æN­q+«¿êT@([‹8¿ïÿ˜ßé#AGNbcu@{Žï²-LogParabolaPMN J1830-4441?ïÐø?'ά$#‰?wƒ¸Ió•?'ά$#‰?ï{ø´å­ø? E¤nǤh?€é\k	? E¤nǤh?îì?%Q@?˜m™Y¦–?®a<ó?˜m™Y¦–?ï0b(ǧý?}	t5'b?™óºà+È]?}	t5'b?驪øºm?ŠX	eá/?†^ïÌ?ŠX	eá/?ìO0ûܕÿ?Á™W²÷í?½†x!P
?Á™W²÷í?í¹Ž9œ·d?£
ý8U¸?²3Ž4Òß?£
ý8U¸?ìËZµ"]?¨|'âEMö?¹§%*S]?¨|'âEMöAGN3FGL J1830.1+0617@B"}@XGßèˆjÀ8³È
Jk^À;	óžÈ®?ë‡	t¦x®@Éý &¼@â.Ÿ¥¢;¿Ü's'Xi¿Ý·íø@˜÷¿áÁ¼öƒ"¿æ¨GúÀ{AGNfsrq@žO­w1ÅPowerLawTXS 1827+062?ïþ°Lc…á?"Ú[ü¡?$û7è>Ó¡?"Ú[ü¡?ïaÓ¡)|?¥üx'â?"Å‹Ý:Ѓ?¥üx'â?ï½xF?~mŸR¨>?€¡ùj\»¨?~mŸR¨>?ï÷
Y/?3_¿ší|$?QäýÌCAù?3_¿ší|$?ïüF4ö4ƒ?>
u
Aë?=ÎVDLœ?>
u
Aë?ìÞî"á?éïŸ'?¹؍Åâ?éïŸ'?u+Ù«?Šr)QØÆÈ?Š\b¸y1.?Šr)QØÆÈ?ïë³´;Ë!?Y/-ò,ö?dLK¾µ~ó?Y/-ò,öAGN3FGL J1831.0-2714@]ä ()ÀÑkÕÎ(À9§™¼ÕÀ;1«.íSU¿ØäƒÒï@IA;3²µ@°ãŸø†¿é"çN5ö¿àÔs·þ¿ä¹¸w͎`¿á'.ohAGNbcu@Ÿ=¨>BZîPowerLawPMN J1831-2714?ïÙ¾½•wK?‡MðCŒ4?s ¡S€êN?‡MðCŒ4?ïJ	õˆ?´t0öL_ð?Ÿüö»Q²ø?´t0öL_ð?ïRêëh:É?zQAövh?•¢¢Ñ<Þ?zQAövh?ïóOIƒ–?E(ŒßQ\?Yam_CŽ?E(ŒßQ\?ïWþR½?›³a–ÈÙÎ?•ŸWž¢m?›³a–ÈÙÎ?ëöðG?ÅKJ=»Í?À$?âáŒ?ÅKJ=»Í?î's&á?£—¯þõd?®îVè͑÷?£—¯þõd?ï.cª
I?'(§KÛa?š3Š¾Vß­?'(§KÛaAGN3FGL J1833.5-1033@5'° F\¿ìU'?Æ$ÎÀ7Bo§WÈ>À9öáP?óæ¢̙¡@B¤ë1g@#ßâSG¿æɸµ™¿ã"ݧ)hô¿ç>EžMf¿è–¥ôEãPSRPSR@Éh$xPowerLawPSR J1833-1034?Ë/:w?̈'6æÏ?é41\»º"?̈'6æÏ?×Át˜r?ͨ6l›C?ä~E³Æõ?ͨ6l›C?ÚÇVmlau?·½n45óŸ?âœTÉIÏF?·½n45óŸ?äoÕöõÚ?­F~žÔ\‡?× TÄL?­F~žÔ\‡?œà!ýш'?¦÷?ª}î?ïþïè8l?¦÷?ª}î?´\îd~L?¼†'ˆsì?ítb3bW?¼†'ˆsì?ÒZb<ë?Áœ°UÙâp?æÒÎöaŠx?Áœ°UÙâp?Ç5W^Øö?¬À‡Àa?ê2½ê(IÃ?¬À‡ÀaMIXED3FGL J1833.6-2103@(UΞ^$yÀÒBß·7À5ü#ü^ŠÐÀ:bÁ'ïV?ÿ,ý|BØ@ ø1T‹È@†Ó8¡²¿ãæ‡Ä–µ¿çWȋA«¿çÍ~d´à¿éZïŠfö¯AGNfsrq@s"Q¢£YLogParabolaPKS 1830-211?ïº{Y›/y?'Ê/MEd*?a)•™©?'Ê/MEd*?îäQ2o
q?¸ÉÿÇXÁ#?¡ºìÜ~ôç?¸ÉÿÇXÁ#?ì:§›Jì?«C*ã]¦Ý?¾*ǃ%¨ ?«C*ã]¦Ý?ïýÜì¡ö­?#DÈ6Ìq?1™òMáã?#DÈ6Ìq?îçHÑø?ŸlXFQÃÎ?¡Ù»}?ŸlXFQÃÎ?ëNBUm£?ÊÉ! Óc"?ÂǶöªIs?ÊÉ! Óc"?ì"Mz1I?«e`-Çv?¿ke".u´?«e`-Çv?ïþ¬‡¡¹=?$gŽ)x?%7†ß'b?$gŽ)xAGN3FGL J1833.9-0711@8‰¡_`¸§?âðÐ $ž×À7øUŽU™À9¦''ØÛ?ÍÂkä™@¡eç»eœ@ÙþÀ9ì`¿ÐÁaߙ¿äŽ8ýÍu¿¿æ†BCÇU¿ÚõâûbatOTHERspp@¶Ðú^5?}PowerLaw?ì¤]ËôEô?Æ]aýB'Ô?ºÝ ]Ðb?Æ]aýB'Ô?îðe8%?µ‰hæ´¯"? ù¯íKÝ?µ‰hæ´¯"?アM-–w?µI–¶ù{?Øú»e¤Ó?µI–¶ù{?ïúGDjƦ?6C"'½?Fâï?"´?6C"'½?íºՎè;?·)1À?²/9R>ã¬?·)1À?ëip÷?É¡Z¶…?Â[çú<$?É¡Z¶…?ée¬ü'¥H?²HëÚËÏ?ÊiL
¹jß?²HëÚËÏ?ïàÚ~ü?ch@âN?où%>'«ß?ch@âNAGN3FGL J1834.5-0841@7HT`ªdÿÌïû_ :ÍÀ7]öÌz—vÀ9ئ²†Ði¿Û'ÝèÍx@-Ì^'Ýh@]é jƒ¬¿ÐP´ƒ)댿á¶`]Õ¿à'¿zÔ²t¿æOó]ZNOTHERsnr@¡:yÛ"ÐåPowerLawW 41?è|Gö}?ÌMÜIv?ÎÒà&	Ä?ÌMÜIv?îüΤpì?³ùý6Rö"? ?³Ý
F?³ùý6Rö"?ââÌ0£>'?µëìÏÃï{?Ú:gž¹'Ý?µëìÏÃï{?ïöíÉò}?PáޞZÅ[?Sè$«SÕé?PáޞZÅ[?èèÿ`¦f?Å©õ'´?Ì\}feÃ?Å©õ'´?냮›çÛ$?Èb…¾ë\?ÁñE`"q?Èb…¾ë\?è¿ï¡¸÷Ù?²[ZoHs?ÍAy ?²[ZoHs?ïª'§ Õ?|Ÿ+'Nt8?…\÷Õ?|Ÿ+'Nt8AGN3FGL J1834.6-0659@8ÍtŸå
5?àºÇà˜ÿÀ7Ã6ù'PöÀ9ˆ2芘u?"2ÛçYz@IŸæ姺@cߣê¿ë.°:Ê?ÓN˜~çf¬¿ÝV¦?oV¥¿à­èÛ÷OTHERspp@¾öPA‰7LPowerLaw?â!|sæN?Ñ}®2öÅ?ÛÕ½3d?Ñ}®2öÅ?îìW?"$?´ýaYÖ÷?¡:Œ';Y?´ýaYÖ÷?á'FÇÇÄ?µ¼\¸}²?Üûrqâpx?µ¼\¸}²?ïâyFèǪ?d£ΰPb?m†¸ð¼¶?d£ΰPb?ççÀ{…²\?ƶ£AÛd?Ð0ô›H?ƶ£AÛd?ëÔ~-=·?ÉÓU"ØXW?Ü®K	$?ÉÓU"ØXW?èzÕ	mx:?³'0P¢&R?ΫÚJ?³'0P¢&R?ïRRì2ç?†®ÜÑñ‡"?•µ¢j¡Õ?†®ÜÑñ‡"AGN3FGL J1835.4+1349@EÇç@™Å@#}1(ùÀ9ÍMüUyÀ;@'¿aª?¿Çâþx§—Å@Ä¿6@¯r_Ãßé?Õ	j¤Zp¿ë'_º6'¿à { ŠN£¿í¨Î¥êà´AGNbcu@QkC,¥PowerLawTXS 1833+137?ïÁΙ"Ø?€``þˊ?³ƒ;ÿ?€``þˊ?ï‰;gÜ?¡¤OW»"¤?±&›É?¡¤OW»"¤?ì]˜×§Ç/?¦Mkÿ¾¢Ï?½9BÁƉ?¦Mkÿ¾¢Ï?ïÝAE‰eß?Zµ)ƒ	?q_]$Ÿ¤Ò?Zµ)ƒ	?ï©;œ•S?8Œ§"+?…±êœ;l?8Œ§"+?í9ÕüÿÎ?Á¢rr?¶7!NÎ'?Á¢rr?ì›E>+<w?¦µÎzDë?»%Ö¦E?¦µÎzDë?îÊhŒ‡S?"n¯ÓEK‰?£YwC&Ä?"n¯ÓEK‰AGN3FGL J1835.7-3258?øß}ž¼C=À&¾S‹'À9áB'[sÀ;¨±gìxd?øN{ÞÓ@ñæ"©r?ð2^צÅ|¿Ñ×Öì
¶¿Ý•»~ã¿éœolŸe‹¿ïÿ\×qk}OTHERglc@'Y["Ðå`LogParabolaNGC 6652?šsé¶ÜXX?¨:B©ÅL*?ï,`²- ]?¨:B©ÅL*?ÁWš4ë?̶úÜ[?ë»*r܅?̶úÜ[?ÔQ·`\"´?´q©)áN/?å×$Oѵ¦?´q©)áN/?ÉÛ=?ò?­p§Xå?é‰0°ƒ|?­p§Xå?‡Íeå<NH?•ŽP£!%ì?ï Êh¢‡?•ŽP£!%ì?¥µT#,z¾?Ãé8×üšŠ?½¿yä?Ãé8×üšŠ?ÃVÐï•?°èw¤Ü€º?ë*KúÄ»?°èw¤Ü€º?'¤]]r?'•Þ}ìp?ïrß.Pd?'•Þ}ìpPSR3FGL J1836.2+5925@V8tÿñ½G@8ÿ'¿°"˜À5<³»ƒÏ-À:YÌÅ@'@ oa6Ò@Րà?õ:€nû5k¿¿NšlÓ=¿Ûʬ"y
¿æ*Ü#,¿î¨Hî}ÃóPSRPSR@‡^áä÷eþPLSuperExpCutoffLAT PSR J1836+5925?òÚnð˜?"Þ³oòš?ïÿ oiÍØ?"Þ³oòš?±øâh£)&?ÃþÕnÃu?íÀã²Â_Œ?ÃþÕnÃu?£‰Î¶¶ÿ¿?œ¢{­"äÕ?îÇc]–D?œ¢{­"äÕ>¸}°t~7.>³ƒàYŒH?ïÿüð+ À>³ƒàYŒH?<´É
&O¢?3ƒä4»–ƒ?ïüifº¸è?3ƒä4»–ƒ?ž½@Л1¡?³y&¸t§Ò?ï
ùD,³?³y&¸t§Ò?©"ìFê¿	?£r,¡-?îfÁ;ZZP?£r,¡->'f‰iñÞ>š3ªª("?ïÿÿtóO¡>š3ªª("PSR3FGL J1836.3+3137@N/sßË­@0É'àÙìÀ9_Ñöy}À;t.QZ¿³ˆœ•N;@Upõ¶@ÅxÀ01K¿è"¼R"®ù¿á†¢®7­¹¿æοë+¿äÅ4
^ôAGNbll@'Ót¼jPowerLawRX J1836.2+3136?ïÿN	«Øê?,¼R$?}?>Ë^&6°?,¼R$?}?ïә›$¼«?'ou9QÐ?v32Yb?'ou9QÐ?ïÉSþÚ»ù?u¤s2Ýß?{V2g¥?u¤s2Ýß?ïûÊ^Ö?.4äWû ?Cû­|‹aœ?.4äWû ?ïýwúYð.?6`Má?4@-jľA?6`Má?î…9èPƒH?¶žèö¿‰?§¬ay?ý‰?¶žèö¿‰?ï/S@Uí?•_ØsBC§?š—ð5Ø`?•_ØsBC§?ïÒtöïX?k{ë±[©?vþE¡e?k{ë±[©AGN3FGL J1836.5-0655e@9áj("?Ád]?Ô´ÖÀ6ñÖ³Ö\À9K~Íey¿õ«µPy@l«…Th7?ÿv
`:Ó;?ïŸíp±C¿ã2dkºc>¿ä5»wà¿ÐÞC\vyOTHERPWN@¿â?²-PowerLawHESS J1837-069?ä
Łî›î?Ñ{s—¡?×ätü"È#?Ñ{s—¡?ïAåqÎa?¬'U{±ˆ?—ÃQÁIé?¬'U{±ˆ?âqŠOx"?µwž`ío?Ûëaýù?µwž`ío?ïÿÞü"þ">ùyˆfÞ>ðÉ©Õët>ùyˆfÞ?ênn©g(>?Úò_-?ÆFEZc_?Úò_-?ì}pn°•g?ÄN=ùØ?¼|Š{TÆ?ÄN=ùØ?é¸aµ
?²(:˜Ð?É{¥+·Ù?²(:˜Ð?ïþ£…;ú¾?+8±œTo°?%Ç©ÕÓÃ?+8±œTo°AGN3FGL J1837.9-0607@9ò€Æ^?ÈÎ_âáÀ7à~SÂõ³À9‡¨ÖM?óêy¶O\ß@ô.·x|¾@"BÀCý[¿ìNùõœF¿×Tj*Kâ¿çfjÆÙ~ó¿çYG·y©dPSRPSR@«)cŠ	PowerLawPSR J1837-0604?½é"ó[p®?Âáë4ýõ?ìBÍa"'ê?Âáë4ýõ?ãÜb™¨29?Ïèâ'Î?ØG:̯›?Ïèâ'Î?×)´¬å?·m]tW†?äk%©÷y?·m]tW†?賉t)ê×?¨±g§À4?Í1Ú/XT¢?¨±g§À4?ž?\³Ëy/?¨ôcš¨9$?ïŠß†?¨ôcš¨9$?ÆÝóóy¬6?É·~ºx¿ã?êHƒ!"ó?É·~ºx¿ã?Ö ­rrû?À	ô¼f3w?䯩FÆõ?À	ô¼f3w?Ör*ú´?¶2'§?äüFêö¦?¶2'§MIXED3FGL J1838.5-6006@tõýç!À5½v Í|À:$Âî&¹¨À;¨¶urrä?íuúÅn@2E³"k?ý´Ü€žöÑ¿â6wM‹Æ¿Ô€[j3ûZ¿Ø3Tq­}¿â€åC!ÆAGNbcu@­ktzáG®PowerLawSUMSS J183806-600033?ïòÍ|õôä?[>ÁÇ?ZeßÜ'Â?[>ÁÇ?ï å'0¨?£A Í)8ê?›ãOÆðé?£A Í)8ê?ï«ôø1vè?<w¸œáÇ?…Áýñú?<w¸œáÇ?îkë *F?""SÿU?©ANåý[œ?""SÿU?ïä"R'®Æ?pŸÓ¾-J°?kl­·
©3?pŸÓ¾-J°?å2QÅß6¡?ÍïœÌ w?՛\tA'¿?ÍïœÌ w?îØ{JèËJ?œèîß?m?¢xKTâç^?œèîß?m?èKJ+GW?¯Ým{?ϊÒ×Râ¦?¯Ým{AGN3FGL J1838.8+4802@S<b?û˜'@5ÔC@ÇplÀ8öïÕ'À;BL¨O??ԟ|EºŽ@¤%D24?üåâDhæ¿ãEÑøGq¿ØýÁ†óyµ¿×bÝÈë0¿ÖŽ¥nRÝ·AGNbll@¨Ñ™=ÙcPowerLawGB6 J1838+4802?ïýÜõÂm?(~O¶ÌH?1Sì÷VI?(~O¶ÌH?ïÏåìƒv?…[OғDÈ?xyŒ÷àLã?…[OғDÈ?ïæ!<ï'H?ië÷OüCg?iÞÃ,U—Ž?ië÷OüCg?ïí¼3©X?Iuà¼~Œß?bCúPgX?Iuà¼~Œß?ïû)?z¥t?@äærÖ#•?C[ïX?@äærÖ#•?îÖÊԜq]?¬ÜÙQ˜ãŒ?¢"R¶8ê5?¬ÜÙQ˜ãŒ?ïÏùµW?€^Ó Ù&h?x}ƒxÄܙ?€^Ó Ù&h?ïþxt
¢?}aƒqœÌë?‹Àaߌû£?}aƒqœÌëAGN3FGL J1838.9-0537@:€o_3l>?Êxßl>À6ŽãðÕÀ'À9>áÃÔև@¦`Ž@
Ì]ÓG?ÿ}³Áä¿Ò˜b0Œ¿åÈmÈì~ª¿ã…j²SŽ¿ìІ^1PSRPSR@©†¥¡ÊÀƒPLExpCutoffLAT PSR J1838-0537?nο™E$d?­hÂÖçžX?ïá1@>ßd?­hÂÖçžX?•5#tã?³ûi§ÀL?ïVVçuù	?³ûi§ÀL?º=ZBZ‡O?©"S—GRý?ì¸T·´¯?©"S—GRý?vß,GÉÿ¦?`Ã9!Ë?ïÒA§{jÁ?`Ã9!Ë?P¿w("4?S{Hn+sK?ï÷ó 1t}?S{Hn+sK?uÇï>4?™q3] P4?ïÔqÄ	üû?™q3] P4?³_º…#J?¯>qÍEC?í"衝'?¯>qÍEC?HWSo<?:cÐR5kÞ?ïùê+P'?:cÐR5kÞPSR3FGL J1840.1-0412@;å`Ÿ}i?â£t?ܨ§À7«À_AÀ9Íúꉯ?õ{*ˆ"¹‹@?­le@Sõ?ݐ"¿âgrÕàqÅ¿èƒÝRu¿æß0$˜;¿ë"Ï"gˆûOTHERspp@–L¬<žìÀPowerLaw?tºÎOt?¡îX@f€?ïÖzŠ'ñ?¡îX@f€?¥:™?<çù?·ÄÅÂA"?î¬Vl1€?·ÄÅÂA"?Ͼ'屮D?±äÞuóuy?è[DÐï?±äÞuóuy?Ê.,Ž(wC?¥i£(šS?éttÜuâ/?¥i£(šS?]:4¥•MŸ?bkÕ{^?ïñbå—7Ù?bkÕ{^?‡p0Ö?§i¿P&Là?ï¢??°ï÷?§i¿P&Là?Ç#2?³yõ=Èý#?ê78:{s`?³yõ=Èý#?–üŽÕr2?fšd¡?ïH‰b-¶?fšd¡PSR3FGL J1840.9-0532e@:ËÂ@ÐO¿Ékd'õµÀ6¦rKPÀ9FS£C^?†è×sñ@ÙÀ»¡V?ü㪟PgÌ?ÖzwéDR¿½EÁ\\¿ÜàÝÓNq¿ßϓ¼
êOTHERPWN@Âôc÷ÎÙPowerLawHESS J1841-055?ìGaÔcø?È‹Qq%¡?½Äñ\à;ü?È‹Qq%¡?ïçݪH?¯ØKŸÕa¶?œƒ»³±?¯ØKŸÕa¶?æœÔ¸º.?´ŽôN‰?ÒÆVŽà‹¤?´ŽôN‰?ïørr,?Iµ±, þ?O†66é$?Iµ±, þ?îåIaY?¨–6í弬?¡«ié'P0?¨–6í弬?ëç89ò?Ɩ™ê¢JÃ?Àc7óü?Ɩ™ê¢JÃ?ì"ÎÆ÷öœ?©²Ô_/"?»a‰È@K?©²Ô_/"?ïáwÅ@?f57ö«Û?nˆ:Ë$Ðs?f57ö«ÛAGN3FGL J1841.2+2910@M8"€,á
@-É0ŸÚü:À9ØÏL
ÑÀ;`,ÖøŸ¹¿íό‰Š@
Ž¨'ƒ?ùóÀ+©§¿ê2þÄZ|<¿áÖ©Ôò'‹¿ãijù—03?×ûîwUnAGNbcu@Æ|·l‹C–PowerLawMG3 J184126+2910?ïý´ãÄW€?3¦™ñ÷)?2Xâ]蔨?3¦™ñ÷)?ïÔ¬ØÄ/x?|òë s2À?u©"¹e#â?|òë s2À?ï½ðez¥…?qÖê¯?€ƒæ®e"­?qÖê¯?ïÿî"eŽ->Ý3AVüÚ>áݯSbëÙ>Ý3AVüÚ?ïö‰Dóá?W¤+"šY_?Rívmt•?W¤+"šY_?î·p˜µ?²ì[öG†?¤ˆÿt¨?²ì[öG†?ïq×Ýh»?6lo?'Åb'""?6lo?ïþapnŽ9?1î¦Ût¿c?)èýu2N?1î¦Ût¿cAGN3FGL J1841.7+3218@N¾'?ßéà@/úÖ 2¥oÀ9J±ÓLBÏÀ;i»Þh¿ðôFn#t#@¿nëE3@v>ËLo?ÑÑ£=S¿è¿èiÜ̳¿Ý9"ûƒƒ¿ÈYÀÛÒÏAGNbll@¤¢N¾ß¤@PowerLawRX J1841.7+3218?ïþSA=?"1 ΁®?&úÇïÖÿÜ?"1 ΁®?ïÓ㙏U?謏0?v35•ÅÆ?謏0?ïÖ~¾eś?trõŠ@K?tÀ ÓL~@?trõŠ@K?ïÿØhiÿV>é/VÏAbë>ó˽À">é/VÏAbë?ïýÃà?r?0¡—"Õç?1àþfÔÁÍ?0¡—"Õç?îß S~ú~?°¹r6…!?¢
úʤ
?°¹r6…!?ï­–TÕ?…–Tû
öõ?"¹šuIž©?…–Tû
öõ?ïþ+†€1?/o¢_¤?-Gœ¦ïË?/o¢_¤AGN3FGL J1842.3-5841@u?«ºÀ5Ë{_ò®ßÀ9È*"yÀ;~¾|§ñ?ÒCP@y¿@
»?ÏM?û ÷ÿ«q]?îÓ
;°bç¿ãÔÃRis%¿Æ[h…`¿Ý
7+÷eäAGNbcu@·«Ø>BZîPowerLaw1RXS J184230.6-584202?ïþ5²`Ý2?1uÃN¤†?,¤Ùá<?1uÃN¤†?ï¨jŒÿ?š|q"~›l?…åx‹$2?š|q"~›l?ïÝ3Wn?p=Kӌ?qfT×y@?p=Kӌ?ïñNÏú\[?DxÈÌî7?]b`ú­?DxÈÌî7?ïü\B(Í?A¬"uÀ?=í=)um?A¬"uÀ?íà|ôꚊ?½.3Q¦à?°üX=8-?½.3Q¦à?ïËO0Œ1I?~szŸ?zXg¨¹OË?~szŸ?ïÊíõÂ?f¸·6 š?z‰w¹?f¸·6 šAGN3FGL J1842.8+6810@X£Óßæ…@9ÕiÀú)À:-¼±Ì–FÀ;¬à‹Ær@¿ðiö¾¸¸@wd/¥µ@jrà_Ý¿ãgŒ"S¿é´µÜ<ε¿ãNtžîî¿âì?œ€²KAGNfsrq@ŒÔ1Ä2ÊXPowerLawS4 1842+68?ïÿõè
Q#>Ф‹ý‹cˆ>Ô0¹f ­>Ф‹ý‹cˆ?ïÛ?ÂÉÏÓ?'7ÊÎÆ#G?r`'Zæf?'7ÊÎÆ#G?ïôÉ;Pk±?P¬dAà?Vm‰d§þA?P¬dAà?ïÿØ­«ŸV>ã»È!N»>ó©gŠÝ4>ã»È!N»?ïÿöf½èó>Ô1ÑI<Ã>Ó2«<£§>Ô1ÑI<Ã?ï39؋>Y?§é۵Ϯt?™˜Äë(˜Ö?§é۵Ϯt?ïòc©êìë?\çá-ˆu™?[8¬gº…?\çá-ˆu™?ïþ$¼*›¾?(_ätdÒý?-´<ü4
?(_ätdÒýAGN3FGL J1843.6-1114@6
€_5ð}À,ß?ëþ@À8¥
¿cíÀ:š`' ×?ò— rç(C@DO‰€ï@ϔÀkëa¿áyÁùCñ¿êi¢'¿ìþ]YÙe¿ïÿzö…ÍPSRPSR@1Ù¾L×IPowerLawPSR J1843-1113?ÐXñ£›Ñ?ËPuŠv?çӇ.2?ËPuŠv?´[™ák~ú?ÂGšå/Ui?ítŒÃ·A?ÂGšå/Ui?ä´@äC-t?³ÏKIöü?֗~7y¥?³ÏKIöü?ÒöÏn'?¬%8Ûª}?æÀ˜H¿??¬%8Ûª}?ºK\y†?ÁûI.ƒ?추pÝ/=?ÁûI.ƒ?™±(ô™Y(?¶¾ãÍfÈ?ï2v¸v²?¶¾ãÍfÈ?Ü2aãô?¼±97H•?áæùÏp†?¼±97H•?™"YšpÇ"?ƒºO+•9Í?ï6í3cs‡?ƒºO+•9ÍMIXED3FGL J1844.1+5709@U­aÿÏX˜@7z—¿¤ÆÀ9»J>³‡À;ÃhEc·_?Â%¿Í_ïª@Ó¤'UÛ@\ 'F¿¿áê£Åê0¿ã3xV¿ãµÝúòz¿ïýÎ xµ7AGNbll@zR½<6PowerLawTXS 1843+571?ïÕE,ìƒ?tIwþ¡S ?u]iqAŽ{?tIwþ¡S ?ï¾Ëœ˜s÷?‡›mmçp.?€MÜú¨6?‡›mmçp.?ïAHt¸å?Ž"' Ti|?·Öùÿéb?Ž"' Ti|?ïtKžäÝ?t)Ý3Rã?'vŒôÂ(?t)Ý3Rã?îo>ãòþ?¨R-¤»Ò?©Ã-)?¨R-¤»Ò?íÍÔkŸÛ?¸´jt¸Å¡?±'\ â/­?¸´jt¸Å¡?ëՌ·^¦?¯×·Q<=?À©ÏÝ"…f?¯×·Q<=?êWü]g?±4i'ܞï?Æ ¿æŠc?±4i'ܞïAGN3FGL J1844.3+1547@G&	_ûZ@!RaՈ]À8ºë"ùÀ;µ}û®b?èqP¾ù@'L(!²,@9v7]d¿Ùnÿmš‰¿×¦on*ˆ¿â›®rÕÆ­¿â W·³\AGNbcu@¡¹týó¶FPowerLawNVSS J184425+154646?ïö¶÷^¬ð?K¦Õd‰?R'šœô?K¦Õd‰?î«8¿?²KáÈ
?¥L~BWÔ?²KáÈ
?ï~V¶ß¿?†wy#†?‹àjAA?†wy#†?îGß7Ï`?‡<ý¦"WÝ?«ƒÆò¥õ?‡<ý¦"WÝ?ïŎ™Ø¦?zyŠöŠ¬?}8³
}¨ã?zyŠöŠ¬?èx7.Ú"?Éõô©O?ÎÃ#D—x?Éõô©O?ît‰Q¢ßé?Ò'ß¼ë8?¨·jæ­èi?Ò'ß¼ë8?åúÉE"ðÏ?²Ä¢‡=œ?Ô
mtÖc?²Ä¢‡=œAGN3FGL J1846.3+0919@DX[_¢'@j!€-aãÀ8l|ÚF2À;$î?
\@üɦ&Ž@Mn=p3?îe@×\?¡þöÉ(0(¿³',²Ä¢¿á±Sißl¸¿ì…0-Å5)PSRPSR@›×ɅðoiPLExpCutoffLAT PSR J1846+0919?R?sÁÄ_.?Sè=@PF?ïöàF½ø?Sè=@PF?£ò'rnY?¾]ö?âÄ?îÀ×ØæØß?¾]ö?âÄ?£h"Þ±Â)?›®é÷z×T?îÉv±ë¨Ž?›®é÷z×T? ÌVç?…_ÝòJF?îó7
¿\Þ?…_ÝòJF?[d¥Ã1ç?Vˆ(—ö™¶?ïòpM£?Vˆ(—ö™¶?'ä—¶îÓ®?­xKËml¹?ïpÛBdB?­xKËml¹?';aì3ch?ÙýH%ïº?ïv$ð'è?ÙýH%ïº?yè=!és?h>ý¾Ÿžÿ?ïÌ/ÁÂ5M?h>ý¾ŸžÿPSR3FGL J1848.1-4230@vó¾ýÀ1cŸVqýÀ:)+rt'À;ŠS².»Õ?àAšƒhC¥@
n¦9R?ÿ8ÿ€SLƒ?ï2_zÜ6š¿ã¡[Dý¾¿Ùd¦ÙÚ8¿åb©a§~£AGNbcu@¬ç*=p£×PowerLawPMN J1848-4230?ïþM|¤Z,?0Àf
¸¢?+(3™®?0Àf
¸¢?ï_å!¬´?¡}ëS¥¸o?"Në1'?¡}ëS¥¸o?ïÁ7èq?{/:(¬?7ãÿhàO?{/:(¬?ï;êaˆ0;?}¶×Ĭէ?˜'³ÈÀ³?}¶×Ĭէ?ïðÑÃùáÐ?eö'*|_?^\wàA_Ð?eö'*|_?ë+¶¹ÝSO?Ãu7ŽRê?ÃQ%Š²Ã?Ãu7ŽRê?>«µ?Jî3üf*?ØpffÞ©?Jî3üf*?ëÆO'ý©?¤¹²EÇf?ÀçæÁô	Z?¤¹²EÇfAGN3FGL J1848.4+3216@Oˆ M@-[ç^jÀ8&	Ñ:×À:_ÙuQ»´À
˜wDŽ¥@p'º}ý@JÇ?Åí¿éªî
¾à¿Ü&âå4o¿æ´Ô¹]⽿äVžÙZµêAGNFSRQ@›?ƒä%¯PowerLawB2 1846+32A?ïïy̎}K?q9O N?`†3u¢=]?q9O N?ïÔލ$ÒY?úˆ¶Œ2m?u¹MJæ?úˆ¶Œ2m?ìÃ@ïxb?©ñåh­œ?¹åÿ"<ï?©ñåh­œ?ïÿÿÿv¡>..M7Úú>ÏçC¾—>..M6j
¿?ïÎ,åU?Št ±}öW?xÿé'ÔÑ"?Št ±}öW?îöÿãq÷6?°&(bé'ü? ɼs¥?°&(bé'ü?ììÀ@³Š˜?¨Ðâ:…'–?¸™ýø=éÆ?¨Ðâ:…'–?ïÿÿöVM>g*à5ê>Suãqs»Ñ>g*à5êAGN3FGL J1848.9+4247@RÁð`P@2{_L–²À:i»dgÀ;¹ZúøYC?èéQ×|î@ G"g{d?úV¾|'¿îÃò¯Ø¿ÇJÀ©º	b¿éµ¶¯]Ò?åwÈ/üiAGNbll@ÃçûƧïžPowerLawRGB J1848+427?ïùâo t??Mj`ür"Ù?HvC®.R?Mj`ür"Ù?ïÅM›$šO?–ËõˆïŸ?}Y2nbÄP?–ËõˆïŸ?ïxJÒ¿³'?…Ø
âZ—j?ö¥¤™ñ¼?…Ø
âZ—j?ïô`Ïp¥?TdÚ³Î?W>aaß6?TdÚ³Î?ï­¶¢úýs?…†oþèT?"'WD°?@?…†oþèT?î*è","w?¶¢šC¬Šà?­Q}Ý6¸Š?¶¢šC¬Šà?î±CŒû.?¡Ë –ß'?¯ôëÆTf?¡Ë –ß'?ï¢,+Ý?¥|V6?ž+ºjŠèp?¥|V6AGN3FGL J1849.2+6705@X_[íöé@9
` ÒŸÀ7¼0íޕLÀ;)ÆΆ
q?øÖ)vò@8t1Bî@ðwy‰-ç¿Þã)ß]¯¿ä Ì=R=\¿ä]ŽGoÄù¿æàS*°"íAGNFSRQ@ð.æ1ø¡LogParabolaS4 1849+67?ïý5bø?JOÅ$¦t?6Tð!
8?JOÅ$¦t?ïÕÿTÎ'Z?…±B‰­¥?uU~ÏKR?…±B‰­¥?úHÓP?‰Ë
ãv.?ŒXmË,?‰Ë
ãv.?ïÿ»Í~¬>ó§ßýàü¿?™ rÏE>ó§ßýàü¿?ïýž	°?4àÖ¢?+Î?7t_aW?4àÖ¢?+Î?ïT_¹à?±JóÑý`?ž5tÃüw?±JóÑý`?ï9>aSpÚ?•ˆhN/ÿE?˜Ø3×I²¹?•ˆhN/ÿE?ïÿÑ°G—*>ù,ªzý7—>÷'é*NÅ>ù,ªzý7—AGN3FGL J1849.3-1645@1³q¿_üÀÀmœ@ÔÀ9Ö®8HÀ;=Øwûº ?çºõ¬¿ç@
~ Lf?ù°ŠŸ*Ó?åUc¬En¿ï÷Š9™­?ïÿ}'Gÿ"¿Ú	ÞxúE_AGNbcu@Â&§ï²PowerLaw1RXS J184919.7-164726?ïûIЌ'Ÿ?GÚâFY
?BؾÛäï?GÚâFY
?îã$­&"?°JYs"t(?¡Í¾â™áÀ?°JYs"t(?ﰗ;ÊÜ?èeÙ‡o?ƒÚ8ô|ää?èeÙ‡o?ïå8‹â¡Ë?j{MºÒÇ?jÇs߅=?j{MºÒÇ?ïä#1·î?qرM"ò?kÜÏ!±?qرM"ò?êç•s+?ÍٚK×U?ÇÄcª3V?ÍٚK×U?ï/¤ûCúù?"€
d>.i?š`—€ à?"€
d>.i?ïæ‡Òƒa?t{ß @Ð?ix-­&ˆ?t{ß @ÐAGN3FGL J1849.4-0057@?Úý¿³ß–?TÜà‹À7½ð÷3©À9¾Ç¦^Û?ø»òː7@y'W'c?ù'cð?m©?ï	Bi1¿Íƒ'[·¶»¿ãµ3S£K¿â¯ò6á"OTHERsnr@«	u%F
¦LogParabola3C 391?ÄaòÝÇ_¿?ÄAx°Àҙ?êçƒHŽ(?ÄAx°Àҙ?ÉkD¶W.?Ç)¹HÞ¿?é¹%.Òj4?Ç)¹HÞ¿?Ûä-§P?¶eó1JÓ?âr
¸i,X?¶eó1JÓ?àÑ´R$'?±ÿ?à?Þ\—[·òÜ?±ÿ?à?¹·ˆ—é–1?¹‹Î'»?ìÉíÍ:?¹‹Î'»?²äÞEØî?¹Ýwhjø?í¿Ãdn>¢?¹Ýwhjø?àŸ—j?cî?¹Å†Ì&M‹?ÞÀÑ+8$?¹Å†Ì&M‹?Êô¿ÃW‹¶?³ßÅÏúÌ?éBÐ*?³ßÅÏúÌMIXED3FGL J1849.4-4312@vx@À1Ú3çüÔÀ9C΋é®À;UÏ2e®?꬝ØB¢@ê#3
ïG@"›€y
¿Ñ¨õRäÄ¿á9£ª¥}¿áҜH[ʒ¿æ—þ7d+ŠAGNbll@›%àA‰7LPowerLawPMN J1849-4314?ïúáÆëª?HD‹R0S?DxãŽ0"Û?HD‹R0S?ïgµ|+Ó ?¡Ã6ÀÄFe?"	P­ó?¡Ã6ÀÄFe?ï¨ "Ò/?…±%»
"?…ù·Ô| c?…±%»
"?îÕdã{Ý=?~Ò·Úæ®?¢©±Éùú&?~Ò·Úæ®?ïâÁÄí©?u#%†À?m>:üì×Z?u#%†À?é°YnR»[?Å)hӗÛî?É>šFµ"?Å)hӗÛî?îÁVI¼?œiª…Ó}¼?£êŸÑ¯:?œiª…Ó}¼?é2¦<Y?¦Ú/Ÿ †Ø?Ë5g›½û?¦Ú/Ÿ †ØAGN3FGL J1849.5+2751@LøÌ?ß @)a ˆ5ÄÀ9µ§íÀ;~¬ 7?ñ5†oE],@ãîƒ*í?@¨8ßðk
?Á—'ӝeE¿äši¿ê!Û®"N¿ë.¿±qAGNbll@+&€IPowerLawMG2 J184929+2748?×ކ~1ß?ÐqìwÉ!?ä¼öÀç?ÐqìwÉ!?äû™‹NJ?Ì NŽ{a?×ÒÌécm?Ì NŽ{a?éàS? ²p?°Ã´âGî?È~³}6??°Ã´âGî?æ>'	#ì?¤Ǥ©I
?Ӄ±íŸ(?¤Ǥ©I
?ªy9 äÐD?²lºJ­è?îXlnîL?²lºJ­è?ÌvY9Ï|?Ê«A˜`ñ?èây©±Œ!?Ê«A˜`ñ?Ò:U!«³?¾ßýVàÀ?æôâÕo*'?¾ßýVàÀ?Æa®-¶ƒ?§l.÷@<&?êgºt'_?§l.÷@<&MIXED3FGL J1852.4+4856@S¦ó?þÑ@3õà_PÈÀ8†oÔ¤1£À;Œ.î¿¿ë$ồ¶Î@˜qB7ˆ@|yÿËQÍ¿â?J«k‡¿å¯uˆ8¿ã‡fýŸ¿á¤mÇr‰¤AGNfsrq@†hî.±Ä3PowerLawS4 1851+48?ïÿÑÌ2jƒ>ñ2¡·ÌË>÷Ir¨>ñ2¡·ÌË?ïÜåŠD"U?Ȩ²/¢c?q:úˍ[?Ȩ²/¢c?ïædµ%* ?sv˜ÑPŠ?i›J›…?sv˜ÑPŠ?ïÿý
²E7>°xˆ::‡>·'IíNDy>°xˆ::‡?ïÿĶX­>÷ù.NJî>ý¤Ô3.V>÷ù.NJî?ï™éº]"?°á»'
)?ŸLÂÊl)²?°á»'
)?ïÌw‡Ã?ƒ=ªßëg?yÄ~–©:O?ƒ=ªßëg?ïÿðá…>áÚ"ÐÕÔç>ßè{èÜMA>áÚ"ÐÕÔçAGN3FGL J1853.2+0006@@€ŸÍA¿Ö!Ÿ¯T¹À7¨R$AÀ9í
ÒÁÙT?þ™ ÍÕá@56B²,@6L,ÔIn¿ápòÁ~%¿çr(+mA!¿êˆyê/g¿ã­_cŠ5pPSRpsr@"q4‡ü¹$LogParabolaPSR J1853-0004?–Ybñªù?¤ÉþÐÐÉy?ïM4è®Äh?¤ÉþÐÐÉy?®͓hŸs?½C'¿@%?îc'.8?½C'¿@%?ÛWÁ®G?¶&ߥE?âTs(Ý?¶&ߥE?Ðc‡ÊöD?®µJ5i‡?çüN<"Þ?®µJ5i‡?¶ ìÁ6™?»¤,¹e?í+âgÏÙ-?»¤,¹e?'Q-Ê1Ÿ²?±'	Åþ?ïuv'×®R?±'	Åþ?Ýb©oœèP?¹†g´ÃaV?áN«H1‹Ø?¹†g´ÃaV?¥¿AW?žÂÉ
±‹¬?î¤á=OÊ?žÂÉ
±‹¬PSR3FGL J1855.1-6008@tþí )À7½F@V1eÀ:Îç·3ÞTÀ;úŒ3‰M?çv1Npj:@›Â[YÂê?ý'(º3?îÀšdoÁ¿ÔÜ	
•°+¿ÂÜú.&Pn¿ß
ZO4y7AGNbcu@´-!Þi­CPowerLawPMN J1854-6009?ïüÊÔ$/	?6<-ƒc?9©\㧾g?6<-ƒc?ï7Ö\²L]?¨}8O|¿ï?™4rMz\?¨}8O|¿ï?ネK"|I?y%AÌ1Ö?€]í'×{¥?y%AÌ1Ö?ïÕBG{?ƒZ!6ÃúÙ?Ÿ¥W¶÷ا?ƒZ!6ÃúÙ?ïónô̽€?a	è'|ð?Y"'àE?a	è'|ð?éŒH–ØÛ4?ÉVÙ«'zC?ÉÎݤœ"/?ÉVÙ«'zC?ïdö1ӕG?©þ°cyf?"a9ōW0?©þ°cyf?ìa^RN_?¦O5Èë·?¼÷ý
m?¦O5Èë·AGN3FGL J1855.1-2243@)½«ÓÚÞÀ%ÙHßlâÀ:IR}ÔAÀ;ˆÙÔLg?ðÖ{<6g@.ÝTYs?ý"ÔÁ7î.¿áøK€±ì!?é€à¶cª¿»-""Ñ¿ä¥wžG(^OTHERglc@·Ðå`A‰PowerLawNGC 6717?ïØÔââì?y&1|€­Z?s•͙Ã?y&1|€­Z?ëÀÏqöE?ÄXj2ü?ÀÿÂ8&ì?ÄXj2ü?îï,fÌxû?—o_yÜ;µ?¡
9'€¢P?—o_yÜ;µ?í›Wü/)Ó?™1Ÿ°#V?³%@`ïë?™1Ÿ°#V?ï.f…Δ+?¤ââ|?š3/A­?¤ââ|?ä'ª"çÔ?Ѥø_7?×Û°ªØ0X?Ѥø_7?íorÁ5r?¥•¹õ‹†&?´"iõ
Éò?¥•¹õ‹†&?êe"ás?¶jš‹X¤Œ?Å¿²iìz4?¶jš‹X¤ŒAGN3FGL J1855.9+0121e@AS°
kù¿ØÙ"`}ZÀ5XôÀ0ÝÀ92ÛŸ'@¬	íI@Ö|O[ÝÌ?üNoVÏðn¿Á~õÔX¿â*ªcy¿æ;êý9|#¿ëvO²ÅºŠOTHERSNR@›¤?åÉLogParabolaW44?ÅZuͶí?Ê1°oQ¥?ê©bŒ½E?Ê1°oQ¥?™ž!,?·"vɼËC?ï7k;®Ï?·"vɼËC?Â)üâ­ùg?°Éz›Aÿ?ëu€ÇT¦?°Éz›Aÿ?kA¾Mšs?oo;¸m
W?ïÁ)|¿Ýë?oo;¸m
W?À™
ú@•?ÇÇÂKêd7?ëÙ½Az¯Û?ÇÇÂKêd7?'6kÒW€?¥bµuÐä?ï·&P‡èþ?¥bµuÐä?ΦÙf,?ŧFš2	¬?èVI¹:&u?ŧFš2	¬?kÞ×ÿX?lÞh5úˆ?ïä!(Tï?lÞh5úˆPSR3FGL J1858.2-2215@+5}¡ŽÝÀ&»Ú@RÖgÀ9'Τ=aŠÀ;‹½÷FóÚ?ý…'MJ@C±Û"Ì?ð³!Ø?ËwúzQ¿ÂŽúPµò¿ç·f'¸¿í˖ìÁôPSRPSR@˜òiÇy¦µPLExpCutoffPSR J1858-2216?b÷֐mêu?uË¥í|P!?ïí)wÑ%?uË¥í|P!?¸FÂj¾?Æ\1sr?ì÷?ç÷u˜?Æ\1sr?¹Ä–ªH_ã?©lŸ¬?ìÇm*¶ô?©lŸ¬?ÊQÝô£'¦?©ú"	Yõ?ékˆ'×–?©ú"	Yõ?R©¬bÿ;¥?Qm/å ?ïö«)Ü>Ò?Qm/å ?¤>Ƌ)?Ày_ýÁŒR?z'
?Ày_ýÁŒR?žÓɅÉ?•N'CÀÈR?ï	a³×»ò?•N'CÀÈR?¡Z
,WY«?kÊ·tP?îê_-HHÕ?kÊ·tPPSR3FGL J1858.4-2509@%ׄABÀoÀ)8!4x®À8Ý-?~À;7é;˜\ƒ?ðÓDá"@¸vb\ìj@Lú¿¤ED¿Ès˜•¯÷v¿èÇON6¿àYÖú¼ãå¿ï	Aš:eAGNbcu@³Ð|"¶PowerLawPMN J1858-2511?ïԂtu.?xîrFÀïú?u¾Åá•ÃŒ?xîrFÀïú?îbU®ûÔ?¶°aš'Uc?©Ú¥Ü)¼?¶°aš'Uc?ê$"ä ux?¯Þo)·,?Çm¬m~*?¯Þo)·,?þBè?½…[Çð{?¤æ"†w?½…[Çð{?ï×êܓ{?sêžNG&S?t}Šœ±?sêžNG&S?é†r),
?ËÀ?͸n?Éæ7[OË´?ËÀ?͸n?êÊVÂÑä?¯ƒ&vÈ?ÄÖ¤ô¸ñp?¯ƒ&vÈ?ësQ^‹³?«ˆ-9ÙI?Â2º‡¥Ñ5?«ˆ-9ÙIAGN3FGL J1902.0-5107@u™ûoÀ6c
?ƒ£ŽÀ8}ík¨ÆÀ;{,Ü×ÜË?ýR=›¥@T˜"#@Ä Wì%¿Ð!°¡?w²¿äPàɪ·¿åÇh>Â*¿î9uýˆ+ˆPSRPSR@ƒO [ÀPLExpCutoffPSR J1902-5105? †î§U('?²Ë~}"Y`?î÷'³èÈ?²Ë~}"Y`?²¡'†­ƒ±?ÄÅwq|?í«Ï¯*OŠ?ÄÅwq|?Ñgvï†Ç?³+þ[?çLqDˆ<œ?³+þ[?®îè±}è˜?"'ÎbôÍå?ît¾æ'?"'ÎbôÍå?{ݽ'ð·F?€i¡.cj³?ïÈD…s¥r?€i¡.cj³?šøžõE‰?°Ð¤¡Œ6˜?ï(?KUÔ?°Ð¤¡Œ6˜?±:\It™?¢ym×ï?íØ´w‹-?¢ym×ï?|«o÷ É?pÆ(R}S?ïÆ© •&?pÆ(R}SPSR3FGL J1902.9-6745@t} FÇeÀ:
%@+i:À9~s£eË6À;¾ç!â¨×?à8u_ÜA@Ü¢­¿ke@ÄÛ Ú+¿ãzƒC8[^¿ë:Û}ó)¿å9ËP©nV¿âógŽ¸ÅAGNfsrq@µc^t)žPowerLawPMN J1903-6749?ïÿ}¤¤U?Gc³òÒ5?Kkˆ"Å:?Gc³òÒ5?ﺽ´½½?•›¢Aå¦Ù?P'ØŸêÈ?•›¢Aå¦Ù?ï{b¯Ö$˜?'È	)ۂ?"ª
bÖû?'È	)ۂ?ï÷¹[Œ`?3\CåŸ>Ä?PH2âÁ?3\CåŸ>Ä?ïÿ:c0Úq?—[Á(7?³Ÿ0œÐ?—[Á(7?îfDx]'`?·×^½æÛ
?©›¸uÛW?·×^½æÛ
?ïùȍ¤?˜a@RN®?ŸàÆú†áŠ?˜a@RN®?ïÒ¥!j¼j?cOÄ@e»'?v­oJ¡Êý?cOÄ@e»'AGN3FGL J1903.2+5541@U~¤?åÉ@4‡ŸŸm1À7ÿ®õKqÀ:Ë>³™õà?ôźߺeA@¡Æ¹¸H?÷_~«+½H¿ÙžRÌ£¿ÕŸ=X® ¿Ú´!!sÿ¿á\äÓºãÒAGNbll@—<ìÙè>BLogParabolaTXS 1902+556?ïø`5Â&"?\ú]?N(åÏÝÿ?\ú]?îÖKø7D÷?¯è´<²ž?¢›@x@-˜?¯è´<²ž?íºws»d?§ƲpCú?²,Dfî=ä?§ƲpCú?í'±@Ä@?•+‰°=V?¶Âuùqê€?•+‰°=V?ïó§ùÈr9?ZóúÇ†?X°5bm?ZóúÇ†?ê^ó"¡?ÄQ¢-«£¡?Ƅ3‹­z?ÄQ¢-«£¡?î€äùi8?¢<ʕÃ?§ñ¿ il€?¢<ʕÃ?æp$C'b)?³¸Œ›Šõ?Ó·xÛ;®?³¸Œ›ŠõAGN3FGL J1903.6-7052@tEõŸôýmÀ:'ë ÍjÀ9"=çÂÀ;¤®Zþ‰?å8æg—Wº@¤ý)+@‰mèþ‡¿çxû@Ÿú©¿Þ*Y©ÙF¿å50ûdS«¿í˜™ç2«PSRPSR@ŒH*0U2aPowerLawPSR J1903-7051?êÍ>¡Q
?Ä`ÊrKï9?ÄË{®»Ù?Ä`ÊrKï9?îÓpšê?¦ö¢À&#À?¢Èø	,?¦ö¢À&#À?êp[
‡B?­»ë®-]?Æ>"ƒÕâö?­»ë®-]?ë݉h$=?Ÿ ­jI†?À‰ÛÒ_o
?Ÿ ­jI†?ãn@e~g˜?Ëepæ$À1?Ù#50Ñ?Ëepæ$À1?æ%œ†«LÂ?ÐÞ>¬/•¼?Ó´Æò©f|?ÐÞ>¬/•¼?ä¤ÖÍ'?¸5ztá	?Ö¶Sôe²?¸5ztá	?Õ­Æ"tÛ/?·4¥PÁjl?å)îŒh?·4¥PÁjlMIXED3FGL J1904.5+3627@PÕlÿݛQ@*˜Ý ·0À:HŒŠ½À;»©°h8?)z?¾´?@
*)Ö=8ñ@ÉXŸÿ9\¿ïÿó´ÿH?ïþIãñ#¿âޔ`}Kä¿ÛýëJDAGNbcu@¢Òñ©üPowerLawMG2 J190411+3627?ïþÑî0?'<šYÁ?"áwâwÔ?'<šYÁ?ï¹ÙØ£ð‹?‹Y÷Û‹?‰‰æzE?‹Y÷Û‹?ï׃Ñuò?lWñAïä'?t>SââÚ?lWñAïä'?ï̟<4¨m?fà#í¡'à?y°aáŒA€?fà#í¡'à?ïû™©^ވ?>0—jO?A™ZàU
E?>0—jO?îJ‰™?µä|ö"?«Wn:–

?µä|ö"?念Õe‰?ƒÃ–Pº†½?†W:'…ÕÁ?ƒÃ–Pº†½?íé>¨1aø?¥	†f‹û ?°¶
¾tðB?¥	†f‹û AGN3FGL J1907.9+0602@DúÀ%¿ìÔT@(4À5ݜ©'žÀ9êXR§lÁ@.[ê¡õ@ÿI@eË·@$̦·9¿Û²oË·Es¿ãfCo°+¿å‰¥ì@ãþ¿ìëè%óôPSRPSR@‡¤p¾
í)PLExpCutoffLAT PSR J1907+0602?g0ÙÚÛè?tš‰òEL?ïèãÎñë?tš‰òEL?˜™öëí?µ0>Ðäù-?ï;0H®UÏ?µ0>Ðäù-?±ÅOΉ
a?¥Àj«Ôám?íÇVX?¥Àj«Ôám?`g›BW½¨?S]ŽV¿‡C?ïï˜d÷a²?S]ŽV¿‡C?[Ç~A?«?_¼ýº"Á?ïò@íì?_¼ýº"Á?}áÞ­!? ýÞW‡Ó?ïÅü<bB&? ýÞW‡Ó?¯M.hA?©XrçwJ?î{/˜–\?©XrçwJ?@µˆ©¯€Õ?BÔ	Û¼z?ïûҝµ÷¸?BÔ	Û¼zPSR3FGL J1908.8-0130@@ÇûÆnåÀ9±êFÀ9ªð]ˍ2À;²g†÷Öf?øçj@
ÌiûqOù¿ëyÖ1iH]¿ïqªôy¨Ò?íåO[¿æöË,¨nb¿í™\ZHö¿AGNbcu@¡'c×
=qLogParabolaNVSS J190836-012642?o<¸gñô?®ñVs¡?ï|†X=P?®ñVs¡?´ŸlHPòN?ó…öF?ílv¾ç÷?ó…öF?ǖ–7—úf?±dF™ G?êZrg?±dF™ G?¼ºpºäS7?°¡¶Cy?ìh±è£u™?°¡¶Cy?›ô¨ƒÎH{?»7¶(¢?ï Z»¸Rl?»7¶(¢?•×Å8Âm?«CAJ"Ä?ïQAÖäþ?«CAJ"Ä?Ân²:O\?®wÙ8<ž?ë{$Sql)?®wÙ8<ž?‹s(Ëä
?‹ƒæàç?ï"ò3AS?‹ƒæàçPSR3FGL J1910.7-6000@u"§e4À9žÚà‹ÆrÀ9ÚïÅYbÀ;Æ{…²\?ô£D",î@ÄáÖõÈ@š½ …«¿ä»Û®ã¿Ù·°ÛÕ~L¿çæ"gÞá¿í»ûÄ1OTHERglc@"ß&L/ƒ{PowerLawNGC 6752?´
|¯›<?·eñ"¯'?í~\ðN¹?·eñ"¯'?ÙÏy?‡?Î*…ËœÙ?ãCþà=?Î*…ËœÙ?䎒¸åöP?³Š¨¦W7?Öâڎ4a?³Š¨¦W7?ày&ž`?ª!Û2p^›?ß
ѲÃ>â?ª!Û2p^›?ždš´K̇?¦5©Á@7å?ïÛ*]¡œ?¦5©Á@7å?·lá`<2?ÃÌRd·÷?í}œþº?ÃÌRd·÷?Ð
—05?´ÁV?fè?çóy4|çæ?´ÁV?fè?´…TFò?ššŠÐëúÁ?íoUÛ¤Î?ššŠÐëúÁMIXED3FGL J1910.8+2855@N{À?ö@!ƵÜê&À:8ðvö£À;€d%C†h?é{noc)	@
~†ܖ?÷jŸÁ%ú¿çZÝ÷lˆ"?ïÿª,cä¿Ùd¸&'B¿²¸oÕrZ2AGNbcu@ÇÌÝ`A‰7PowerLaw1RXS J191053.2+285622?ïýõ7z??hܧRª?7ÐXÉ$>??hܧRª?ïnãØ>V?¦wìã¨w?'#œJŸ2?¦wìã¨w?¯K~ü?ŠOТÅ<`?‰RTò5"?ŠOТÅ<`?ïœÚ0¸"–?uӇ®D?ˆÉsÊÿ¢u?uӇ®D?ïõÊÿ1à?S*Odº:^?Tj¶™p³?S*Odº:^?ìÆdžJ ?Ã~~Y»÷×?¹ÌÛ…¯?Ã~~Y»÷×?ï_&q?•ÌðÎ?">xJd^?•ÌðÎ?î§,:'?¡Ä™ëE?®eŽ>ã?¡Ä™ëEAGN3FGL J1910.9+0906@E ßÔŽ¿ÃäH~ôÒ¥À6k3æÉÎÀ9–M$v?ú´'ÇÅ&@¡NÇѐ?ÿk"Æ(˜Ð¿ßc%  ¿ä\áýál¿àUf.2Br¿æ´7À
DŽOTHERsnr@¤[=ÈKLogParabolaW 49B?È}úPWu!?ÈÁ{±gm?éàkê"¸?ÈÁ{±gm?°ðZv'/L?ÀªyRs·ª?íáô±d³Ö?ÀªyRs·ª?Ûn>Ìï\o?¶ƒ'C B?âHà™ˆQÉ?¶ƒ'C B?Β´
'±÷?ªÉcEž?è[Rý["'?ªÉcEž?°eÃr=Ý?³JˆëD³Ã?íýóG­5$?³JˆëD³Ã?'£'•1«?¨j$GCG?ïrãkŽˆ2?¨j$GCG?Þá(
ØmŒ?ºyü'È
?àkú"É:?ºyü'È
?«"¿‡m[É?—¼ä]žQö?îF´À$?—¼ä]žQöPSR3FGL J1911.2-2006@0â
_ÕR­À*sç_JHÀ7ºÚ4"\À;Êʔ
i?óusºaæ$@´›Ü¿ß@E¸7~¿ä_Œ+Hk¿å¯rÎ"`¿æԃâu¿ê]8ÉÛxAGNfsrq@ƒ[Ñ¢£YPowerLawPKS B1908-201?ïô³~OÅ?TD	<eF6?WҘԥƽ?TD	<eF6?ïBc!u?¨¦ÛgŠ|?—³s:Vµ?¨¦ÛgŠ|?(œ"Ø?–ûWx±j?¤¶
uaë}?–ûWx±j?ïùEÜÔ?5‡1ÖW?KŽë
€÷ý?5‡1ÖW?ïÚnÅW°?q±ÑéS*ž?rÈù•Å?q±ÑéS*ž?í'Uë€'?ÀRG¼haÏ?·vÅQåÄ?ÀRG¼haÏ?írË"	?¡Õª2æT?´i¦ðkε?¡Õª2æT?ïô¹,uÄ?QÖŒ†N?WüöËhg?QÖŒ†NAGN3FGL J1911.4-1908@1ÑŸ>õÀ)½ôafLeÀ9j+Q½aöÀ;6dE#ö?£7.aߐk@"î´þúÇ?üQ¦áUÅÚ?ïµF2`Ǹ¿Úá–|y<¿ÒèÛµ ®¿ÖŠÛÞ$AGNbcu@¶p´Ý/ PowerLawPMN J1911-1908?ïû‹+C?=I5כÆA?AÓTý;?=I5כÆA?ïO« œ?ªÓNUG?–
‹ñ¦¦?ªÓNUG?ï¼E¤1‰?{äÛgìa¶?€î¹	å¿?{äÛgìa¶?ï÷J¹b?9åâ)؁Ä?QÃÇg͌˜?9åâ)؁Ä?ïîùf¢'?]ö^'ƺd?a™Ëð·?]ö^'ƺd?ìð"ÂÇæ?Ã&m¿˜~3?¸{ƒÚW´N?Ã&m¿˜~3?ïI"ƒ\ì?…ÚvGsËÃ?ˆ­žìç4Ý?…ÚvGsËÃ?ïÚE8÷ËÝ?fåäìk]?rÝc|ŠíÀ?fåäìk]AGN3FGL J1912.0-0804@<	I`œ"
À }ÖOÀ9~ø&²òÀ;Œ#QA¿É¬v|DZ@Z¼#jR@\"Ý¿ëÂÏÏÐQ+¿ÔÎ)¦cú¿ßrצQ'¿éú–«õßAGNbcu@š Ä›¥ãPowerLawPMN J1912-0804?ïᔥ>Š?wöÿ·?nkZ‰"Þ?wöÿ·?îø±W%€Ã?µ&DX¿? tꍧóÏ?µ&DX¿?îÈOP0€7?™_Uo†?£{C?™_Uo†?ïû[¼?,eÁÔ·8?B'ߪu¹?,eÁÔ·8?ïˆ&Y}l4?'/è>ÜùZ?öi ¤ó?'/è>ÜùZ?ìZlÄ4³ø?Äd¥'AIˆ?½,™ÞZ`@?Äd¥'AIˆ?ìáþRJ%?©Šª0ž6?¸ðÞ·‰X?©Šª0ž6?ïâûä2'?af1Hˆ–"?mûë²æÔ?af1Hˆ–"AGN3FGL J1912.6-1223@8+OP À$‰®ÁIÀ8Ú7æ÷~À;!•ÄøÿÓë!Ùf¹@¹ø`Nt@ïÜÀŠÊ¿çƒÌZáøÙ¿æÃqù[dï¿ä8,ŸÎÅ¿âñn±}UAGNbcu@†_\=îxPowerLawTXS 1909-124?ïÿ¸f'@%>þ$$—sÔ?æh$ñ>þ$$—sÔ?ïa#ÒÄ?¥],8¿¥w?"ÛŽ¼­p?¥],8¿¥w?ïÙ×äFÕÁ?uQ–Þ"×?s
飣X?uQ–Þ"×?ïýuJ"Ê?"	ښât?4WÞÓbW?"	ښât?ïÿ8V~+?Î8æºâ,?ýöøNyÀ?Î8æºâ,?íRÆ݅½Ö?¿¬…ë£ñ?µiɈ6Ó?¿¬…ë£ñ?ïÀre<´?'Ÿ7ÐM$?ÆÍwù&?'Ÿ7ÐM$?ïêgpR~?[YîZÍì?e˜íïd?[YîZÍìAGN3FGL J1912.9-8008@s <€"ÞÀ;c¿ÂùÀ8²gˆ¥UÀ;CE?¥1}?÷õýR{¢ä@ÿÿL%óZ@il(¶X¿àøm"—ø¿âøëÒݙ4¿æ€;WM¿êŸ½¨ %AGNfsrq@Š¾?]xLogParabolaPKS 1903-80?ïÚ½ˆ·:?xFëh­"?r¡;¬
?xFëh­"?ïÁSé¥åF?ŠþÎÕû?VE Ç?ŠþÎÕû?Ó?š]ìt{àž?¥d.W1ô?š]ìt{àž?=Wò¸Í?e4Öo7™=?€ØªÑ,§?e4Öo7™=?ï@tJÙ?•/þH»rÂ?—ñvªuAÈ?•/þH»rÂ?î(]T¢wA?¿>­òŽtÅ?­z*µØ‹ê?¿>­òŽtÅ?ë"pôEü?®ž	¤pA™?Á®<.ëŒ?®ž	¤pA™?ïWÃÄC
?† ¢1Ï£?•‡wœÞa?† ¢1Ï£AGN3FGL J1913.0+0910@EÇwàmò¿â:þ Œ=À7éç3ö¨À9ʜcxu]?ý"T¦uu"@
Eq•n'®?ýiš¨¸E?ïÿf#dLõ¿àñfœí1¿éíM¦¯ŠO¿înÂÛ(ÒPSRPSR@ ¾ÅoPLExpCutoffPSR J1913+0904P?4HAZ‡?Uü¬WÇ;?ïýv÷"\Õ?Uü¬WÇ;?¦Òâ U?Áªx}Ùä?î'ÑÝò}Ð?Áªx}Ùä?¨'ªUJP?ž^NƵÒ"?îvåZôS‹?ž^NƵÒ"?³dÅ ó$?–-sŒ?í"g[·il?–-sŒ?0ë¨Ïº÷ú?9QŎwÏ?ïýâŠèë€?9QŎwÏ?ƒNòè{*?Ÿ%i@íMN?ï²Ä4;µ¨?Ÿ%i@íMN?'ÍÞ
Zù€?› cvÂ/?ïi'v.t?› cvÂ/?‡Mª"ùð?uZ˜HkÁ?ï¢ÉUkcÉ?uZ˜HkÁPSR3FGL J1913.5-3631?óA« §UÀ3å*?nªÙÀ9·ä$gÀ;qBÖ>f?؟ºoýéÐ@lôÂ4B}@K^ tT;¿ØÎÖ1¥i‡¿åNGÉö·5¿ãaà·);Q¿ãÜQFAGNbcu@™Ï˜y=ÙPowerLawPMN J1913-3630?ï´x™¢\?¸qsØçM²?'øäå-?¸qsØçM²?>ãø?™>ÇÞGëÉ?ˆÙ0ŠÕñ?™>ÇÞGëÉ?ïvÁ¢ø ?'dBU£?''˧Üóù?'dBU£?ïÿŒê#?_Ø?ÎR9œ?_Ø?ïÿ¢+RX?·¾ Ïê?u0ª"w?·¾ Ïê?îÀ¤lÔ?ÁDѯúGô?¯ÖóôdÇ?ÁDѯúGô?ïl)¥J?'Éb cVI?'zß©¥(º?'Éb cVI?ïýœâ¾'?)‰OÃ$Ü`?3êgQoÍ?)‰OÃ$Ü`AGN3FGL J1913.9+4441@Rö+`Ø@-÷™ÿðæˆÀ9úâénÄÀ;ª
ájÃ?Ü<<
Lo@F¯ÀÍe#?ýužèó¿å07õËÛ¿ÔúòàæN¿ÔÔߜC~@¿Óž£:†§AGNbcu@®C½¿HÌPowerLaw1RXS J191401.9+443849?ïý yišÆ?D<*°Z?6ü3ÒÜí!?D<*°Z?摒µ~R?"Š6|'?…\: ^ۈ?"Š6|'?ïÔ8ÂÐZÝ?r49öúPq?uãžy–©?r49öúPq?ï't:%ô?pB<Äa-i?‹¢øç'¯?pB<Äa-i?ïð»7о?_¡{y–Ä{?^‰'VTƒ?_¡{y–Ä{?íÑðÅr?»kHV
±L?·Qr1¢o?»kHV
±L?ï™]ĬAè?"Z¼')§0?‰¨ŽÃÁz"?"Z¼')§0?ì
Ícu›?¨b"!¸?»©"äS&?¨b"!¸AGN3FGL J1915.9+1112@FÙIàâi¿Ñ._ܒÀ7ý:8
2‰À:;i…Õ—w?üÐ=‡Êå@‡žT"Vå@6ßïiYá¿á­å_—¿æÄ
¡C²¿è>ÓåÅ¿ïþ—ëC°YOTHERspp@N?b¶®}LogParabola?¨îMÃ/Õ?°¥;R9Ô?îáZÆÂ?°¥;R9Ô?¤bÜߍ›i?¾ªNêì?î¹Ò2"£)?¾ªNêì?Ôµ2Y÷÷?µ cĺ?åø%fÓ?µ cĺ?·Õó3ù2°?•úÿf!ÿ?íA™Ž˜?•úÿf!ÿ?'þzøL`	?±Ãs¹Ûå?ïp(=?±Ãs¹Ûå?…1)%Çä?¥´þÔÁ*?ï«;[\q?¥´þÔÁ*?ÆR§·êg'?³)òúh(?êkVf?³)òúh(?†e+ÑÅ#?o˜—7ªìF?ï¦k§Bú|?o˜—7ªìFPSR3FGL J1917.7-1921@2<‡`±ñÀ,§Úáb†À8'Yáó¥À:Îÿ€¾?ãÊåÁæ?@'"T±I?ýòÓÿñè:¿É¨còÿ͑¿ÜøÉkI¥¿ÝF*ú¿ÚÙ©Ê>R AGNbll@¤7ÖOv`PowerLaw1H 1914-194?ï÷ñ~»zs?QãøÔýÈ?PiF?QãøÔýÈ?ï^"	6¬Ý? i¾ý½þ?";¾à	œ_? i¾ý½þ?ï'F	"î?Œý§.Yd?‹®xÁ
`|?Œý§.Yd?﹕"Ùf?cù˜æmÁ?~£5Y-?cù˜æmÁ?ïé§@¡/æ?c8ŽZèV?fX¿Lò""?c8ŽZèV?ì«|Bú.7?Áòáýi*o?º¤è.ŽD?Áòáýi*o?îÝ(«å?œL]H'›?¢-uI§?ª?œL]H'›?î×±¼Èj4?ÎpSÂp?¢"ä0å§Ä?ÎpSÂpAGN3FGL J1918.0+3750@Qqb¿è¸¼@&äÔßÀÅXÀ:jå€!ùOÀ;ÅÃqÚ7ï¿ûŠ­ Œ§ï@j£¼2K@‰_²?¿å_Á¤$·ð¿ãÞOªüÝ%¿Ø¡=6÷ì¿ã«ìE@¯{AGNbcu@›—ø7´¢4PowerLaw1RXS J191810.2+375315?ïþgœqeH?2ê'"?)†<±=zŒ?2ê'"?ïÃáµMeu?'K%×Ò{?~%t9€?'K%×Ò{?ï×èÙÀ³?oøTÁ¬í?t"-°¨?oøTÁ¬í?ïÿÒ¨ÙÓp>ìªçö>ö«•Z҉¯>ìªçö?ïüùàMªz?6"ÿDÅ?80ýe—µ?6"ÿDÅ?î¥ò˜ìÔ?¶¾xLý?¥ ÖnŸ
–?¶¾xLý?ï¥WåÇ?"Ó†i)þñ?†ªº‰r=?"Ó†i)þñ?ïûnZüzå?DH6uŒ/?BF"r"£Õ?DH6uŒ/AGN3FGL J1918.2-4110@vL» 1ίÀ6=QÀ¼ôÀ8ŽÄ¾áQ¿À;E%£þw?ù®:m$¡@Àn&nª?òÕ5 É#J¿à;Y2~àä¿Èì0g"/¿ÙÖwø×d"¿äü/Ö(ãpAGNbll@š'ü¹#£LogParabolaPMN J1918-4111?ëÎUž "?Ãíu]‰?ÀÆ©…}‹z?Ãíu]‰?ãn6>€nO?Ìiq0¢gÒ?Ù#"'ÿ#a?Ìiq0¢gÒ?åCË$Ñh?¶Ÿì{8¼?Õxi·î]/?¶Ÿì{8¼?äð"o6?®Uª1Í?Ö×É!"ñ?®Uª1Í?ãYí(¯C?Ð.Z \ìÀ?ÙçL%®¡z?Ð.Z \ìÀ?Éûµì>4Í?ËɋˆÎŠ?é"ðrÍ?ËɋˆÎŠ?çp}oÜÀ?³–ôýo6W?Ñ GÀ€?³–ôýo6W?Ò,ï@Ó?³–\,¹Œø?æéˆô_–?³–\,¹ŒøMIXED3FGL J1921.2+0136@B㭟àÛxÀ‰¦ ¿çÀ8Ý^ʐ²À:û( °z?à÷èόš@…#Ôñ^}@º 3§!¿çg.ÀæBG¿Ø¿›¾Ycì¿ä`U£ª?¿í!5ÜI±>PSRpsr@'‹½¥PowerLawPSR J1921+01?Ü®l''Ê{?Î~RºÑ¼e?á¨É¾¶šÂ?Î~RºÑ¼e?ëW$—9#?Æ2[fË?£m££u?Æ2[fË?æàÄy¡Ø?²<Ç­£ô?Ò>x÷¼Q?²<Ç­£ô?ëB÷ ˆa?¢•C%r?ÃÒô#}Þ}?¢•C%r?Á0b•ÃÄ?Á%Ÿ_½?ë¾3çZ?Á%Ÿ_½?Ù¼‰	Jú?ÒX{ó|  ?ã!ÿ»{Zƒ?ÒX{ó|  ?àM_ãÚ^?º¢éRÙ/ ?ße@8KÃD?º¢éRÙ/ ?Ó!:›:G?²Ç"µSâÀ?æob²bú\?²Ç"µSâÀMIXED3FGL J1921.2-1232@8ô¢€Èè<À(u¡ueÀ98äŒÜòµÀ;A_~Ù?ᓧº[(@b~Ù$@Ihßg"?ìíbM@êE¿á-V>>ï¿â2Çc½{¿ßڈíÇCAGNbll@£hð ě¦PowerLawTXS 1918-126?ï9"5Š?À¬È(*ôÿ?ŸýXÚ€Ã?À¬È(*ôÿ?í"UAI?º6ºÝrâ?³_T?׸?º6ºÝrâ?ï2TxIµ"?'t²"w™?™µpûðų?'t²"w™?íÚ¿9øZ€?"1mÃúV£?±*2bíz?"1mÃúV£?ï!"lU‹?šKU+)<?›Írl·–ã?šKU+)<?ãŠÆÛ¤´ˆ?Ðé!Òã'?ØêrH¶–ï?Ðé!Òã'?íäú%J'J? þ<`;Q?°Ø.Öa,? þ<`;Q?ã²÷ù÷'i?¿6C]ö?ؚ±-?¿6C]öAGN3FGL J1921.9-1607@5´ß¿ØÀ+Èô^â
§À8ý»V'ÄÀ:òéû±¼¦?仍_Ø
v@V;mê>M?ùØÏY§f?欄ñì†?ËA~ÂRË¿Ø	žBI¿ÏjØïx{ðAGNbll@¸<×â'@¸PowerLawPMN J1921-1607?ïóñ?"
¢?RôCÊ2PN?XeÞ:º?RôCÊ2PN?ï
çb‹v§?±‹ÃZAÆÈ?žCµpc
?±‹ÃZAÆÈ?ç›&¯?…[¬°Þ?Œ[FWQ?…[¬°Þ?ïÔߟk?\ùoöfm?uùø}¢f¡?\ùoöfm?ïÐöù­;É?sÐXîVÆ?w"ƒ,Ñ·q?sÐXîVÆ?íz	‡¶?½¥–kւ?·/¯ÆÖ?½¥–kւ?ïKˆD0m?f!£çñÙ?–Ž÷h҈k?f!£çñÙ?ïxúÁìbÙ?'ÑÞBŒµº?à§Ë
ªÔ?'ÑÞBŒµºAGN3FGL J1923.2+1408e@HŽá@!X?¿ÝŽ™¿óå.À5É'm,SÀ9'Óˆ¨°Ž?ÿdF0eùY@ñÔÌËu4?þ«äÐ(Í¿Ø3)˜—¿âÏ^w"›Ü¿âÐ¥Õ>í¿ä®ÀýᗵOTHERSNR@•IùÀëíúLogParabolaW51C?Â
%ŸyF?ÁSÞH%v?ë|¶»Ø!®?ÁSÞH%v?«]uôEY?À˜}@XÆÒ?îNJ( »ª?À˜}@XÆÒ?×ë½èMW?µ|Ò®¹'?ä
!ñÙT?µ|Ò®¹'?Á²¾ª[nø?¦–³—8ïŸ?ë"PUi$B?¦–³—8ïŸ?¾çtIËH?¾½v}"\?ì#'vƗ?¾½v}"\?'ΤN–G?ªƒ¡>6n?ïqŠÝÐ;}?ªƒ¡>6n?àÀ"wy3H?¹w´ÃEÙa?Þ»
™q?¹w´ÃEÙa? ¯.¼Ý?–¥©Q°g`?îõ
)q'?–¥©Q°g`MIXED3FGL J1923.5-2104@1.¸À¦MÝÀ0A'ÿùJÀ7û:Þ"_¦À;1!àûX?ýÎrn²eB@EÍNY?þ6¾¾P¤¿Ø'#_3¿áñ"þÏÿ1¿äay¯XŒ¿ìÒÖ{™ ÈAGNfsrq@…"D2ÊW¨LogParabolaTXS 1920-211?ítÈEöÑ¥?¶D¬2WÔ?´Y½ÏÛU?¶D¬2WÔ?ïm©.jª!?¤>ÏÚ¯t³?'JÚ0òíò?¤>ÏÚ¯t³?áN}úµEû?³?Ÿ'Ñ\?Ýc
•t
?³?Ÿ'Ñ\?ï÷†vsœ&??)ì§?Pó‡c@??)ì§?èŸjØJ¸?À*ÒåHLS?͂WüžÕ ?À*ÒåHLS?í1éÌâÇ5?¿Ÿ÷I֖X?¶p±—1øZ?¿Ÿ÷I֖X?æø­Ñ½€?°Ÿåoþ7?Ò¤\"ÿó?°Ÿåoþ7?ïùÅÑÂ?HìÈœåø?KÄèí1β?HìÈœåøAGN3FGL J1924.8-2914@"´ö€$}ŽÀ3œ`ÔV.À8+¨¶mÀ;@)8Þmß?Ó÷#óC@0ƒ¼7©:@F¿×ñÄ¿äVÇâØ'¿æ^òŖû¿ç¶1<¸íó¿å-«eã£mAGNfsrq@€9£Â‡èPowerLawPKS B1921-293?ïÿY2ÞØ?¿Ã
¥4?Ì^6\·?¿Ã
¥4?ï'PE+?¢Mmíªy!?~+ò$´»?¢Mmíªy!?ï«þD‹m?"ç«Ae?…8nÝ$Ö?"ç«Ae?ïý«ô(ö?Þå&F0?2 ]™V͸?Þå&F0?ïüþéÞ<?=J‡(8u?8±§y«@?=J‡(8u?î%Ó׶"X?ºÒÙgv?­¢Â"–Ê?ºÒÙgv?ïR¨ÔuÇ?'{à…˜.*?•ªåmîË?'{à…˜.*?ïõRš²?MˆAÎ*NQ?U[ÜîW´æ?MˆAÎ*NQAGN3FGL J1924.9+2817@N篟•\@kDß­úûÀ:p3SêÀ;~ۋ¬q
¿ãP¸t{'@DÖ(–!?þ$º_ÿ¿ïÿûZÔ·Ó?ïÿ'IÏ_'¿Ý©ªFB¸¿Öt¶©R|ØAGNbcu@³ñàuöýPowerLawNVSS J192502+281542?ïÿJÀîr9?Ú_ãá?§ÛxS¦v?Ú_ãá?ï±£÷¨?"änyç>ì?ƒ—98Ï?"änyç>ì?ïá€ñŠ¥?lA3Ø®M?nüS-Š¹?lA3Ø®M?ïþzއN,?íÙRÎáæ?(R䇀G?íÙRÎáæ?ïþ|Aïä?$îr"™ç¤?(;ß$‡í.?$îr"™ç¤?îI0䵇ó?¹óu
̕M?«lñµƒgÑ?¹óu
̕M?ïÏT[T˜?yìk?=~x?x}UéØ?yìk?=~x?ïòó²6?ú?T>Íf>ê?Z›Çºñ?T>Íf>êAGN3FGL J1925.7+1228@Gõ¥À‰d¿üw'áC§JÀ8'rϏÀ:lêÔЦ?à¨I¾B£ò@ëºùe²@Øó_ތé¿×W}ê*o"¿éÊhó‹Ë¿çF:*.î¿é.ð^ÞmðAGNbcu@‡b®±Ä2ÊPowerLawTXS 1923+123	?ïÖÃÜ
\Š?|õ"r\;/?tžPzù?|õ"r\;/?ï><÷,FÛ?«AMÿLjÜ?˜8a.ò¢?«AMÿLjÜ?êxÏCÁî?±äWápüJ?ÆÂðøGœ?±äWápüJ?ïÎ4¾£"D?[¾MØûÚ,?xå ÄãI¾?[¾MØûÚ,?ï_úB%9?ŸºTämY?"··œ ù?ŸºTämY?셩þý²¯?ÂتË	?»Ò°jˆ?ÂتË	?é7Éäÿ¸K?³sræÂæF?Ë ØlÓ?³sræÂæF?îÞf§Ë=?‹%'JÕc?¢•'ÎÏ0?‹%'JÕcAGN3FGL J1926.8+6154@WS*`%څ@3½¬ÿ§ëlÀ8ªlÞPÀ;6w†IZ½?ñB%)[.@Ó;.ª7w?ýÓÁ`]ö¿Õ2¬inÈN¿Û;¿¦@Œ¿Ü4…²uÍ¿Ô¥R?=¾AGNbll@¨øŽ}VlôPowerLaw1RXS J192649.5+615445?ïÿRÕ?%{µe1?½@÷uÐÜ?%{µe1?ïÀOUӜ?‰õY2÷#?ØUã¡?‰õY2÷#?ïÂÁÙ'?véïÿÙ?~Ÿ7'+?véïÿÙ?ïƒz
b>9?m Ÿt{Z?!|§pqØ?m Ÿt{Z?ïÿr6Ì? ¡bEJÕ?^ðæ[á? ¡bEJÕ?î
¡˜øH?·]D*Œj?¯%ætŒÆ'?·]D*Œj?ïn:´m¾?' Á[ô?'8©k~B?' Á[ô?î"ˆk?›)«òxB?¯M×yNž?›)«òxBAGN3FGL J1927.7+6118@W0€5D…@3mù³>†À9'&µvoÀ;€‡6À†m¿óؑÇ=@Ó@ÑÌf rý@#oÀbV¿ä=¾bb¿ä
ËHp夿åQ ¤®SC¿àÏ	ñy0AGNbll@•ñ—Á½¥PowerLawS4 1926+61?ïüø_]ï±?5bUa½©~?8=Ò0!?5bUa½©~?ïÙ­4[
?ìWÄôy'?s)tÚ#ͽ?ìWÄôy'?ïֆ]bíÇ?vËw1į?t¼Ñ_·(S?vËw1į?ïÿµÃN|m>ý#Zifà>? ßâñ>ý#Zifà>?ï÷·HE?RÄc% g?P'o&E
w?RÄc% g?ïþ֛hã?²™â€…yç?Ÿ %1ºMž?²™â€…yç?ïQʮ˖'?'EX°¸rŒ?•Æª-ls?'EX°¸rŒ?ïù±G©.?H‰¬k~?I;Ҵӊ?H‰¬k~AGN3FGL J1931.1+0937@GÍÀÓgÀ0î#;nÀ7þÍ;,&À:­?}ÄQ?É@-e²"@縨ã?ýà Éc·¿æœò1¾Ç"¿Ø?R}r¾Ü¿Ür£»Üdš¿ÖN—+™ûƒAGNbll@ªáç-PowerLawRX J1931.1+0937?ïþKjÀë?,mQ>TÌ?+IPk†\?,mQ>TÌ?ïZ÷	·8ç?©Hö|¿0g?"¡Ça(?©Hö|¿0g?ï!°BÂ6?Šö†$^év?ˆ·"ïOrs?Šö†$^év?ïþdú"ð?«bO?)°[*/ÂÓ?«bO?ïù!#¼Ñ?M"d+¥‰g?K{p_ÿ?M"d+¥‰g?ìê$uo¸?ÂR"¿jž?¸®ÜUc±A?ÂR"¿jž?ï'rì0À<?'öÆsÆÎ?cEŽ`Ü?'öÆsÆÎ?ïú%ä§E:?@̵lnÞÚ?GhmZþÒ?@̵lnÞÚAGN3FGL J1932.2+1916@KR ö½?¹†¿ÉÅaÀ7r?«ºbÀ:Rîu"Ó@‹1:Š•p@õi3JZA?ý"ò0±T¿Û ×æÜBŒ¿åÇÜÞÉ`¿êgž~¿íA‰Ï:ÿõPSRPSR@•UsüPHPLExpCutoffLAT PSR J1932+1916?YQêƒÃû·?gŠÅóŠ?ïóW
ÜZ'?gŠÅóŠ?¦¤>FäJU?Âx'EÎ?h€?Âx'EÎ?Âùã.@¸µ?®nec\?ëA‡4oÑÓ?®nec\?'軜Ja?i‹J_ki?ï´]¨ôÖ?i‹J_ki?[ÔßmFÖ?b$KhN?ïòNÛõ?b$KhN?€g:äón?¥¸ˆ"†?ï¾cCÑ3?¥¸ˆ"†?µG¤±àO?°9ӎYŠæ?íWiÖ?°9ӎYŠæ?P›«fÓx'?A¾fŽœ"ß?ï÷²*Mö?A¾fŽœ"ßPSR3FGL J1932.6-4537@v
…@FA-À9ï)ªIëÀ9—*}'ÞÀ;©ôö·â¿ÜøbøGÏÍ@Wª³|D@ "À@øC¿Ú€²[Ìi¿ëbœ#P€æ¿ÔÑð֟çð¿ïÿí ²Û"AGNfsrq@ƒt¼jPowerLawPKS 1929-457?ïÿ&U¡"‡?0'y›iSß?5T(~?0'y›iSß?ïƚÉou.?›ê4oPù?|²›=ö•$?›ê4oPù?ï2Jï¬:?'rYæZ¥Y?ŸY¶œãÓ?'rYæZ¥Y?ïû·v_"?4§QnÑ÷×?Cù!<ÜAn?4§QnÑ÷×?ïÿizS?!HµLÓå?е€á&?!HµLÓå?î±éޚC|?´^¬~eÆ	?¤ábï}5?´^¬~eÆ	?ïϤ‡M+?••/±ÜL?Ÿfk¦¾²?••/±ÜL?ïÙ+ áC?mñˆO˜7?sj0\R]?mñˆO˜7AGN3FGL J1933.4+0727@F4^ FÇeÀKËè À9Ìò''sãÀ;K®æ1ø¡À47ŸÔq1@"ôW€D‰?ûäÛߏG0¿ïÿöµÿF?ïÿ°²Ô˜¿Ì/'ŠÒÓ¿åSd¹AGNbcu@»ºx"t¼jPowerLaw1RXS J193320.3+072616?ïüÐW	Àã?>W·Ò×â?9}I	ë?>W·Ò×â?ïˆB
ÞÍ£?Ÿ¢mÄ!Ú%?ï}7‹m?Ÿ¢mÄ!Ú%?ïÊU³³¼?vÁ…fžÔô?zÕ&FÀu¨?vÁ…fžÔô?ïÿó¸}>܍ȧ8òú>؏‡|þ#'>܍ȧ8òú?ïæN‰áüÆ?n|Ÿ8?i±vdR?n|Ÿ8?ínVä'ý?¾îë8P\?´HݧV?¾îë8P\?ï'fdc?‡äï9{z3?ffãÐ#¸?‡äï9{z3?ïÿeâ÷ O?•Wu*« ?C›C#¥1?•Wu*« AGN3FGL J1935.5+8355@]ÁÁÖυ@9τ´Ñ.À:9‡aˆ±À<£mWò/¿öxƒ.ž#@"£]'­A@Çó?Ó)³¿èž	㉿à+xÿ›+¿çCú°¿âÚ)nä9PAGNbcu@Li³únPowerLaw6C B194425+834912?ïüÙÔÆÒ?B"Iî¼ç?97Ãii‹?B"Iî¼ç?ïãªoCž?wÏö"Þ¶?läUÔ¹#?wÏö"Þ¶?ï®$'¸£í?{Rísò|E?"vßV¦x¥?{Rísò|E?ïÿœúï>þþLðߛ?ÁkÚ'L>þþLðߛ?ïæ›Öh_˜?q­ŽöÝ?id)­çm?q­ŽöÝ?ï
TþÆ*?²­(ë9R?Þµgr¬?²­(ë9R?Û|Ï?¡5p®tå?¦"ïƒ$
?¡5p®tå?ïòÈQO±?Y»ž9ܲ?Zoç
©­?Y»ž9ܲAGN3FGL J1936.9-4719@uò®ŸðË°À;î€{»bÀ9he˜ºÀ;>`ñ—‡?Îí,öz'@Š+"+ÁO?úAÆa"Ú ¿êü¼Ëfµ?ƒPØ5¿2¿ÕÏ
ž¿ºhÿ{~Y*AGNbll@·k‰ûçl‹PowerLawPMN J1936-4719?ïþ¥7Ã?$œ>wz"?%¬…†{ZJ?$œ>wz"?ï²HEˆ?–Èw7û?ƒmø…Õý?–Èw7û?ïº*j¯Ò?'Icý§Ÿe?ue\!%V?'Icý§Ÿe?ïû—º`'w?*^Ù=
} ?A¡¶¸õ¾?*^Ù=
} ?ïüƒ8¯?>+Ô·óªS?;æ;&}]p?>+Ô·óªS?îƒÂ+Öiü?¶ûê°X:
?§ÃÝFü=?¶ûê°X:
?ïua÷Ÿfì?'Èì¥'?'SÁ
Êð‰?'Èì¥'?ïéà»[?VèL"cä˜?fì 4Ì?VèL"cä˜AGN3FGL J1937.0-3956@vrìà2ÛÀ9SÂÀð À8ÖϦ›àœÀ;y°Øzù?à4èß
R@þÚæëÝ@fë¿VA«¿æ-Råf\ç¿éÆ@ÓH«¯¿çA#5åA¿éó¨—´AGNfsrq@x'ЛùÆ*PowerLawPKS 1933-400?ïÿ4漍?IZÄPìÿ?c0`Ju?IZÄPìÿ?זּAù}8?"òèo‰ˆ|?"ÒowQÞ)?"òèo‰ˆ|?ï¦JŒ[K?—è…¸*Ç?†mxÙy'8?—è…¸*Ç?ïÈÞùþ'É?`ŠöVɑ_?{ƒ	¦:?`ŠöVɑ_?ïþ©vÀ¯?,–½rñ÷ð?%gå$Y?,–½rñ÷ð?íw´sÕ\?ÀYÏ|'?´B[ôÏHž?ÀYÏ|'?ïJ»‹Âý|?'/ž²š>?–¨Ž	J'?'/ž²š>?îQ¦Iïüì?•)ò|:·W?ªå›c"æ6?•)ò|:·WAGN3FGL J1939.6-4925@uÏ¿˜0äÀ;ÜLŸëÃ2À:5¢,RƒÀ;ŽŸ–2ÜÌ?éù·ê¬%@
Ý,µ?½Z?ùüÿ"µb¿î&µ´NÉ?ïþÖ¥œ9æ?žØh-Þ,¿äèòÂÕ¨AGNbcu@¹?PowerLawSUMSS J193946-492539?ïücÝb?I Ú8R`í?<çÐ7Æ¾?I Ú8R`í?ï1þ!òT? ¶´"*?™À>én? ¶´"*?ï¢2»U4?…<÷[ ?‡sxÊK{?…<÷[ ?ƒÒ`?h
þsÚ?¦Uç͋?h
þsÚ?ïõÇZi?h••wJ°?UÊÞ¸Ã¨?h••wJ°?ê™þÅÝH?Æî´©ü?Řè‹Þà?Æî´©ü?ï_&¡Ýé]?'ËĈE?"+DzpP?'ËĈE?ìԟÉ{?´Fk¸ŒƒD?¿q[É´%?´Fk¸ŒƒDAGN3FGL J1941.2-6210@tèWÿ›V2À=…êÀӚFÀ8´wM>w4À;xv̗?íõíqL@§[-M@%@u¿]MŽ¿Û[-3{׿æU™ªû0¿åIUÐRN"¿ì)Ø`Ô¬AGNbcu@†•4mÅÖPowerLawPKS 1936-623?ïë)¾•?g"F©¿¤ï?d€ð¾äÏ?g"F©¿¤ï?ï¹èõÞz0?—1ádäz ?…—¼
?—1ádäz ?îðŽŒ0‹Ÿ?'$§'D+? ÷;?x?'$§'D+?ï؀ø8
ˆ?XY2prˆ?s¿ƒÕŒ_Ü?XY2prˆ?ïæ¦|8á?gù'%÷Bè?iYëEî'º?gù'%÷Bè?î¾ö2ÕGù?²½Zû	‡N?¤œÖj?²½Zû	‡N?íº(¬â??£º(]ÖÆ?².ºŸ
?£º(]ÖÆ?ïg©áª\?Ü·'/Be?"
ÃÂ%î–?Ü·'/BeAGN3FGL J1941.8+7218@ZÁ?ÐÐh@6ÀA¤À9]þÀdßÀ;Ÿö\OŽ?ó'-ªP@L÷¥¾k
@Z9¿¿H*¿ã•ó‹¿è"}š¬ál¿êISäŒ:¿ì–a\Ö¥AGNbcu@"ßèÁTɆPowerLaw87GB 194202.1+721428?ï÷Y¶³8…?LÛDZ'?QL'²L&u?LÛDZ'?îàKÿÚ?¡¿Á`sb?¡ûOŽ€f?¡¿Á`sb?î÷Ù«W‡%?"Áõuü? 'eL?[¦?"Áõuü?ìc`F´á?Å21}ý?¼äýÊ_xû?Å21}ý?ïøjU;ú5?RU\ŽuO?NVªLí^?RU\ŽuO?ç‰í.—3?È×|ÉTGU?Ðì%¢Ñљ?È×|ÉTGU?î¿Nlta?Ÿ ûV°¸Z?¤9'ò?Ÿ ûV°¸Z?àʦE¾??²RØ÷Êɵ?ßðj³tƒ'?²RØ÷ÊɵAGN3FGL J1942.7+1033@HÝ Y§;ÀuÈ@K·À8:Cû"~À:Á'h$¬ˆ?ïÃ|"jÞ@Š)åË?ý¦?Dc‡?¨lÑir¿ÒÛz,Êký¿ÝÍؚ$GÍ¿Ûܟ†K;ÆAGNbcu@ª"bMÓPowerLaw1RXS J194246.3+103339?ïϨ»ºD¤?s¬Aö;?x+¢*lÒ?s¬Aö;?í×5ïÙ?»ŽäŸQi?±FW7«Z:?»ŽäŸQi?îÕm™ֆ?˜z…|:À?¢©&lŠÉ›?˜z…|:À?î)ÝÛ¬¨Y?‰¸@ˆ7DÛ?­b"FíHo?‰¸@ˆ7DÛ?ï:]w»‰•?"HŽƒÓ¼?˜´QŽÍk?"HŽƒÓ¼?æÈ~;š4õ?ͼ¦9™‡?ÒoˆË–?ͼ¦9™‡?ìórϑ‰f?¦—ã¶6u?¸diƒá¨O?¦—ã¶6u?è›(ñ!?²WXîûî?͓\;Ã}?²WXîûîAGN3FGL J1943.2-3510@ƒ/ÀÀ93_ý–™À9"ÞFqÔYÀ;‡^¼Mùˆ¿ÁˆÛrú?ï@b•ZDÅ@Â@+"-¿âÀ'Æ…z¿éèF>ÂwM¿â¸%ÔX¿ïÿʓ6©	AGNbll@•[ ¥&–PowerLaw1RXS J194306.8-351001?ïùôs¸g?PƟ5"?Kà.–FH?PƟ5"?ïŸË`Õnj? ÈPH9L?ˆ
'À?I? ÈPH9L?î›Ê{Ç]?–·N
ét?¦CX‹¼5?–·N
ét?ﲪ%F?l~|.½Z?ƒUvÉôÌä?l~|.½Z?ïñj› Ϧ?nßü¡n?]*Éў"l?nßü¡n?í׸¡zAB?¼°ŒS¤±"?±B:òäp?¼°ŒS¤±"?î'¢ÜÁêú?žEŽGЂ?­…Ò/•Íe?žEŽGЂ?ì²#°«¦Y?¨œÕ??ºnâz¢Í9?¨œÕ?AGN3FGL J1944.1-4523@vAà?pXÀ;ڙ÷LÀ:²ÕíݾÀ;Åëõ‡:?Õ¾°>÷Œ"@
MYÁ<uÒ?øô­ÿ'+¿¿ïSZðç^?Är0ìSr:?¸
K?eè߿ڔcl®KAGNbcu@ʲr° ĜPowerLaw1RXS J194422.6-452326?ïþç¹YŸÑ?&ˆ¤§è
L?!"nU*ù?&ˆ¤§è
L?ﻔ"?"S?Õôaé?ܨ¡š%?"S?Õôaé?ïÑÖ-ëíò?t1Ö^•en?wèíÜ;Q?t1Ö^•en?ïì´S"6†?KD»vY<Î?cK¬­CÙÂ?KD»vY<Î?ïü¯lOð"?;Òã÷Çc<?:"",oþ?;Òã÷Çc<?î¿LlÑK?ºMëa…?¯492ëT?ºMëa…?﶐ÆiäÔ?ƒË´3üÄP?'[Î`k?ƒË´3üÄP?ïº	‹;T?vªyXǀ?}2€ã?vªyXǀAGN3FGL J1945.9-3115@!Ø,àèÀ8"ªKÀ9-Ë)^žÀ;kÇc€À]
ÐXó@àqŸªÆ@̂Ÿ­¿æ¦;r®¿è¹áaÅ¿ØÕ5¿åÍæŽÙ¢AGNbll@ŒÕt!-wPowerLawPKS 1942-313?ïø["â`ï?PÈ햘t?N'¬ÂæÇ#?PÈ햘t?ïÊ¥n¦?‰Ç­—í
õ?z­s‹&?‰Ç­—í
õ?爫ãæfH?'0œå²V"?…†ÿ‡5ô?'0œå²V"?ïÿýAÅÙO>¸¢H»âtÐ>µò±Ã,
D>¸¢H»âtÐ?ïé¸U¶/?ipeMœ•?fþGí¢(ã?ipeMœ•?ïƒ'NÕ?¦8}«ï‹?üφÖíd?¦8}«ï‹?ïÓ½+ïó?—"_D"jÇ?ŸåˆZ'¢?—"_D"jÇ?ïÿ¹Ÿ¯™q?
]Ó
ïJ_?˜Ž©?
]Ó
ïJ_AGN3FGL J1949.0+1312@I«?ÚácÀŒ,ºËCÀ9²A'è|VÀ;A'¡ Ï?àäß@ƒå"¯‹@KxßdÔì?ïÿƒ¯]·Q¿ä7¯JA'ú¿æÌ°i·¿Öý¾Û%3AGNbcu@¤P§y¦µPowerLaw87GB 194635.4+130713?ïûÁÕ«vD?GáÚìK%I?@ø¨mt&V?GáÚìK%I?ïaZö›¨=?¤íÆ\9IŸ?"Ô¡,Šøl?¤íÆ\9IŸ?ïUvT4?"Œyèˆ?œ•Q74‡?"Œyèˆ?ïãoc?V	èé8ja?lœbm?V	èé8ja?ïçl±a¿ì?qŽ™z€ÊÏ?h"Nœà;æ?qŽ™z€ÊÏ?ìA@ÀB-€?Å£0hŸóó?½õùýî"?Å£0hŸóó?íàÿŸ»zH?¥BíYmJ?°øÂ?¥BíYmJ?ïWW:'˜?Š->µDn?•´åvþ?Š->µDnAGN3FGL J1949.4-6140@tò$ p¸ÐÀ>yn Ç‹DÀ:Vû…Fü>À;º%—i=±¿íÕµ‹"h@Œª^¸È@vý §•[¿í5}€¼Ür¿áÄ´ø@'¿×4#H.˜¿êç…-YˆAGNbcu@šwƧïžPowerLawPMN J1949-6137?ïãÂ
s¨?k°HÕU`E?l=€°"×ö?k°HÕU`E?ïÕÔl©L?…iY¦]£ÿ?ur•é÷®
?…iY¦]£ÿ?ïK%Ôa'?•¼ÙÏ|?žv›Hãw?•¼ÙÏ|?ïÿh²éCG?EGr?é©éÓx8?EGr?ïÏßéV'«?}íOŒí?xO7Jm?}íOŒí?ï3'Ýi¨?¬Ì\Ø{µ6?™›Wòh?¬Ì\Ø{µ6?í賵υ9?£gXÆîûò?°ºbQâ¹?£gXÆîûò?ïùµDF2?BÖ×&D¥?I*𼑦f?BÖ×&D¥AGN3FGL J1951.6+2926@Pjå?õ¹U?õh?."À9R"狔ôÀ:é'üft?ö*åS×B@T+ê¿|?ôg ÈÍcÌ¿ßs©$Ññz¿Þ'0",J¿èrNÁÙÿ¿ï9ºHfOTHERspp@›)ÞÑ·LogParabola?µx6¥Ÿ"?ºr
*ó–?íPù+>`þ?ºr
*ó–?ÜM;s.Üó?ό¡£f?áÙbFh'†?ό¡£f?Û¥ÿ7<?´p›¹"ƒµ?â-@1db?´p›¹"ƒµ?á›	Ü!Ôf?³øU¬?ÜÉìG¼W4?³øU¬?|"ف?'Q«!ƒ?ïÆ è¥<Ý?'Q«!ƒ?´«@ÿZý?»˜òGä"Ý?íj—àÔ ?»˜òGä"Ý?¶ÌqZÔ!?§žXCƒ¥?í&qÝy(œ?§žXCƒ¥?¼WAõÁ?§.'ê®?ìuÁ_'Ð?§.'ê®MIXED3FGL J1952.9+3253@Q2	ÀÂl@šñ`*CÀ6œÔÞF.À:›™[†8"@¯A"4Ø@'©«µz÷@Ná¾\¿Õ²Àe¡'¿á(ò"OhÒ¿æ{"噑¿ìèj"U¾PSRPSR@…àL'PLExpCutoffPSR J1952+3252?Ca'K~ì?E'®´ãȬ?ïû'›¥b{?E'®´ãȬ?¤Ìˆ¬§â^?Àè[y',?î³7uFŠ?Àè[y',?¡ƒîŸ6e?—}Z0¾‡ç?îçÎñ?Gé?—}Z0¾‡ç?Bêe%'?2ãÐA®€(?ïû~ivf?2ãÐA®€(??¡òpö&?86™ahåB?ïüË݆?86™ahåB?Œ×ÃËÇ>?«îßÎàŒî?¡5‰?«îßÎàŒî?†•xS¥y?ƒQÿˆØ‰?參òGìº?ƒQÿˆØ‰?ÃMãúë	?£¿T?¥Ž?ïÿ1åf‡Û?£¿T?¥ŽPSR3FGL J1954.2+2836@PO­K6?؀ǿáp¸À6ó®«y•îÀ:QÏng¼¨@æa³Ï$ì@ÎC°.@»ò¯Šq³¿×$Á®"0,¿àËÁcj¼¿å xðÏþ¿ì…i/ˆG¦PSRPSR@'MOßPLExpCutoffLAT PSR J1954+2836?Q¦Ø›ö^?Sº–Å!i?ï÷,"  
?Sº–Å!i?¡Ž#*Õ?½*œ~ÙØW?îçÍ_2¯?½*œ~ÙØW?'ºC†ˆ2?'?&	É?ïwr-Ö
O?'?&	É?sÑ\x®Áå?_£•Èàù9?ïØ]G6}ô?_£•Èàù9?>Û*wáÒÕ?4¯†¡2Û?ïü$š­Úˆ?4¯†¡2Û?‡q"[°ï?©æ¼7(`F?ï¢9®Õôq?©æ¼7(`F?ye.qEr?sÇ[`†M?ïÍ5¢ú…?sÇ[`†M?J-ç->Å?BE雌?ïùt†BWq?BE雌PSR3FGL J1954.8-1122@=¯@Î&iÀ3(¿ó vÀ8d£zÃë}À;Oß;dZ?ó"ýèù~1@eSvŸ™Ž@+"ÿѱä¿ã=/!î¿âÝ@Š´¤b¿æ»j¥Bø¬¿çä¢WNAGNfsrq@»¯ìVÕÐPowerLawTXS 1951-115?ïû,F¯è?D¾Ê–<É?CŸOðû‰??D¾Ê–<É?ïW(úäÑë?¨z[&F…?•à¦Õ^š?¨z[&F…?ïYÞ#	Ö?‹å×SÇ$?"Ä;¢¦/@?‹å×SÇ$?ï±]c;_?cy"+F°ä?ƒ¨§2BJ8?cy"+F°ä?ïæ7;¢åÀ?nä]ìê?iÈÄTÛ0?nä]ìê?í±}!
?Á7¥]È@?·JtÈÒ+?Á7¥]È@?í§ ¿±9?¤\²¢Bú??²Çzù&9?¤\²¢Bú??ïva
ê'?‹Ñœ{‡q	?ž'3á²K½?‹Ñœ{‡q	AGN3FGL J1954.9-5640@uOº¿¹¾ÓÀ>üfß2*À9ø&yçL«À;¬&è¢i?ëáß͟Iv@Iè"Ïf?þ
•µ¢º¿ê³À;ÄÒ-¿æÙ~*ʦN¿Æ²˜£-Ž¿Ð¾cÓd©AGNbcu@°ÒQ&éxÕPowerLaw1RXS J195503.1-564031?ïùrF2X1?Lˆ‰²h˸?J6çi¿ÓV?Lˆ‰²h˸?ï¯èh£q?" ×'VÊ?":Eèîɨ?" ×'VÊ?ï®ÖëgJE?¥x(gsž?"JE·0ì?¥x(gsž?ï£ßüˆù?lân?eÕú?‡ÝÿÜ?lân?eÕú?ïùÃÐFK`?T&Z"?Hð¿±!ä-?T&Z"?ì§
2\b?ÁÁØÕ4£?ºÇw–mì?ÁÁØÕ4£?ï9Ùäs˜º?"Ë#??˜ÄÃqŒèº?"Ë#??îT"É(±?™g	'qû?ª¶Ãk½!æ?™g	'qûAGN3FGL J1955.0-1605@9 1ôoÀ5"
`:Ó;À9qá/Z`ŸÀ;^ꉯA¿à\L'ª@†Õûõ"Q@`=;"¿ßÍã}"S¯¿è2:àÚ(‰¿Ïñ¢Ål¿áû¶¡+"1AGNbcu@¤×
=p¤PowerLaw1RXS J195500.6-160328?ï@°EêÏ?¼6Æü ?—é÷[êØ?¼6Æü ?ïƒô‰ÝÂq?£X²•<˜?݋þÿº?£X²•<˜?ï^‰Žä?'jëxŒî5?".ß%ñŒ?'jëxŒî5?ïögÓxãl?A°<¤?S0X°ÃÉB?A°<¤?ïÀi¾éw?‰¿^ß.Z?Ë ÝíœÖ?‰¿^ß.Z?푘ø΢)?¾g€ß¹d?³s8;B¼·?¾g€ß¹d?îº-âZË?šuى?¤](nM?šuى?Jۊ?€·qSNæ~?ˆºÕw—ña?€·qSNæ~AGN3FGL J1955.1+1357@J^à€øÀ;– oÀ8áú"pmPÀ;6¬¯öÓ1?ï³–&@,ëp{é@é@kU¿ßÿ¦"÷@¿æE9BkàN¿á
ЬÅ	N¿éÓÇùåpAGNfsrq@"s®—OßPowerLaw87GB 195252.4+135009?ïû›énÝÈ?N;¶mÙ²?A[KÞ!—?N;¶mÙ²?ïYhÉd"Ü?«m–Šæ?"Òæ̐,'?«m–Šæ?ï²<KÆä?ƒ,µü_ç8?ƒpíç#Ð?ƒ,µü_ç8?ïäúO´?°?Ic$*ÈÙ?k°k\¸D?Ic$*ÈÙ?ïúV†r‡?Kåáå‰ß¼?F§Þš‡Ë?Kåáå‰ß¼?쑪œ÷,?Ä×Þt{8A?»r«G£?Ä×Þt{8A?î¦ID0? úd¦ñç|?¨¥™³îû? úd¦ñç|?ï¶Øªâ¨g?r<O©Bÿc?'IÕAֆ)?r<O©BÿcAGN3FGL J1955.9+0212@E8"åx•À*ƒõž}.)À9÷Wfï"bÀ;o³1fª¿ó*ü6i@
œs]ð¡?þÖ
€·ux?ïøjb§ó'¿ãC_T	¨±¿â.­*M¹û¿Ó`óí»
AGNbcu@¯"ƧïžPowerLawNVSS J195547+021514?ïýê,Õ)?3Zå_-ø?0®žÔJ?3Zå_-ø?ïi"K‡E?«±3ŸV×Y?'ÏvNj?«±3ŸV×Y?ïÍ\ÁÄRw?r¬¯¼åÎ?yQŸ*åHO?r¬¯¼åÎ?ïÿÈēv>òLcå×>ûý˜D³>òLcå×?ïø܉ ­?Lž^šA‡?LÛ,rÓa?Lž^šA‡?íôðsVJ ?¹°á@č°?°X|f)–?¹°á@č°?ïh²wr8"?ŒH%ٖ?'鱘%œ?ŒH%ٖ?ïü¯'÷‹_?<°tÃØ~?:ƒg¤7+?<°tÃØ~AGN3FGL J1957.0-3234@ "´ ©ÓÀ;4À_×,À9Åþ¦c¬xÀ;€­-¿ãAði\@s³û¼?@§Å_ÆB¿às¬ûԪſïþՇuC"?ï¯d3[L¿ä_Ë~GŒAGNfsrq@|¦"ž­Õ'PowerLawPKS 1953-325?ïý
¥úÑ?GV™2
®*?7«'5!Ý?GV™2
®*?ï½uÂàöâ?'Ø^˜•!`?€¢W8…‰?'Ø^˜•!`?ïz­e~_?ˆˆ ÷&ªž?ªSKµô?ˆˆ ÷&ªž?ïþ§þ6Q?0Ù>•tÙ?'ýў±?0Ù>•tÙ?ïöKaä\È?a¤V	²Z?Si<<pa?a¤V	²Z?îýÞÆ'Û?­gÕTÅO? "ŸEàG?­gÕTÅO?î]u&¦:š? Ha{lž>?ª(­"Ào[? Ha{lž>?ïüo²juë?Sÿ©p·°(?<'kÏP3?Sÿ©p·°(AGN3FGL J1957.7+5034@U&¸`.>@&G^cb¦À8(ÂÂ#&À;täǕUg@ÿ¾Šêª-@ò/@µQÜ@—çZl³¿ÝŒr'¿–¿äÒBR5¿í;u-meM¿ïÿK<igÎPSRPSR@}höݬîáPLExpCutoffLAT PSR J1957+5033?'Ù©'Q?›64=?ïwY7v0U?›64=?©— oF•Ù?¾ÐSr¡eÉ?îf…øýØ3?¾ÐSr¡eÉ?ÍÅm]?±·o:Yôç?莻ä¿)?±·o:Yôç?pŸ1'z b?\_W\þÙ?ïÞÁÞf—?\_W\þÙ?'u2²ó«?§ö‹lm,!?ïtVj´˜'?§ö‹lm,!?–ú+Ò,7?®ºL
"?ïO€.Ê©î?®ºL
"?º½Ì‡`9¯?®/§©Ðê?ì¨FoøÊ?®/§©Ðê?4¯|†á?*íýW‰Ü?ïýj6{_?*íýW‰ÜPSR3FGL J1958.0-3847?ø¿ÜÿŸÝÖÀ<úéŸkj²À8ƒêìÀ;GX&1Âñ?ö/R֑œ @ß*òœë@I1c$g"¿âͺPy¸¿å'¾7³ ¿çe"·'Üo¿ëxû¿S'yAGNfsrq@w¨ÌƒfQnLogParabolaPKS 1954-388?ïÉ9z*é?]õü{c?{cBë›Á?]õü{c?ï'J"r°?§ž²\Xýd?‹­{›#Sä?§ž²\Xýd?î•'ÞJŠ?¡Sq"¬tÝ?¯¦¦Þ«»h?¡Sq"¬tÝ?ïèÀ>&´Ó?OTˆV•?g?Á²ÏŒü?OTˆV•?ï¶hbG¦e?…£23SËv?'eçf/L²?…£23SËv?îÉñÿ>í"?±&v|j&?£`à'½?±&v|j&?í˜Æ¾Eî?¤ETϹ[ï?³9ˁ1é"?¤ETϹ[ï?ïÕÒp‹êk?kŠ'£WÉÆ?uDZθ?kŠ'£WÉÆAGN3FGL J1958.2-3011@%åéÞU‹MÀ:Ǎà'ódÀ9×Ç.'Z¸À;h†`Ô¿©ñ/H;.ß@œ€9¡6q?ý²³?ê•œSÞ$¿æäWôÄɯ¿Â·è"cQ‰¿Ö|âž43AGNbll@·‡§®záPowerLaw1RXS J195815.6-301119?ïÿ3U(6¼?3ãÕ¥€?•_'ô|½?3ãÕ¥€?hzsŸÆ?"¬úv2Ÿ*?€ás–.d?"¬úv2Ÿ*?ïÓyHã–	?~'pL¬?vC['†O^?~'pL¬?ïþkàùª{?o'[ۜ?)AìHBW?o'[ۜ?ïÿIoH?±Áϧƒs?ݖ<ž•Ü?±Áϧƒs?îøÍg"?­BÓnpD? s)ˆ¦?­BÓnpD?ï¸Zq]ä?‡zÄ—Bú?éc­»?‡zÄ—Bú?ïûª5Ѧ¯?:¾@b¢!B?AW)3pýv?:¾@b¢!BAGN3FGL J1958.6+2845@PxèӔ¿Öƒ×`#¬-À7	.Cà)¡À:o9ä'\@æZSÒ@'€ÊjÇÊ?ÿWS–€	¦?<gºNoû¿à`ïë¿ç¨óºÞsú¿ë¬êŸ·çPSRPSR@üoÝëÙPLExpCutoffLAT PSR J1958+2846?i"ñ'ˆ?sÉ{ 2G?ïæükÿ`&?sÉ{ 2G? \¾¶£Y{?»w¡À7EÅ?îú4•Êh?»w¡À7EÅ?©\쒀nÒ?¢5š&È?îj16®½Ã?¢5š&È?gHs1á¨?T•¢~"?ï跌Ò>"?T•¢~"?P'3ãe¢=?J"ŽTcŽ?ï÷¾æ/Io?J"ŽTcŽ?…£ù#TßO?¨zCø³)?ï©p›çÓ?¨zCø³)?z+ü¬?zy¥‡µRÊ?ïËÍÁÇé—?zy¥‡µRÊ?>4X–XV?5®p$ËjÖ?ïü9tÉ^6?5®p$ËjÖPSR3FGL J1959.1-4245@vQð€0<À=üÀu¦uÀ8šw§×IþÀ;~×¢äß?ð5b]]?@Æ&ö¶@Å»à~í¿áíÐGMû¿çB5×Ó;&¿æ`,,¦®¿ïn1–¥ôFAGNfsrq@?–Ov`PowerLawPMN J1959-4246?ïùÛùz6?FC®‹…8?H§@Š?FC®‹…8?ïįÎÓüÜ?–º¦@õR?}¨"¡º1?–º¦@õR?ï³rCûi?ZoHsr?ŸÉ'°¡Zõ?ZoHsr?ïìªËp+a?Lf\Í!í?cU4•SþÌ?Lf\Í!í?ïøÊYk?Oè$Ò¢æ?NÖS÷xá?Oè$Ò¢æ?iy?¹·ôÌÆ?§ykÝ»á?¹·ôÌÆ?îÈ9¹y?™*tÍÑ<p?£|dqÈ	?™*tÍÑ<p?ïƦ3>?rŸª;e¤O?}¼¬Äȵ$?rŸª;e¤OAGN3FGL J1959.5+2047@M—ç@™ÅÀÅ)ÀBеÀ8¾í:*ž9À;2šY²ù½@)ï¶Ü @>2«#æ?ÿbxò)(¿Ò¼·µ}>´¿áæO̊Ìf¿é͉Ñ`Á¿ïÿÕOþ"PSRPSR@ˆúzCþ\'PLExpCutoffPSR J1959+2048?yIMn X¶?'`R¿Ú9â?ïÍmeLúž?'`R¿Ú9â?£|Åà±?¾Ýa
Sb?îÈ?ƒðÝE?¾Ýa
Sb?¸bð,{Ȟ?¥à6qº?ìó¡úU
?¥à6qº?ŸÁfª>?€	HÜ«#?ïWú+Än?€	HÜ«#?j>@ÈìN?w*à›ç?ïåÁ¿
ؗ?w*à›ç?C9Hr â?®¯–N>/?ï'óÐw
?®¯–N>/?"!'ó—?ŽVý•òt?ïfóx{³?ŽVý•òt?f´k-Õ¹ ?Re²hª?ïéK"í§'?Re²hªPSR3FGL J1959.8-4725@uüÒ}ÔAÀ>Û'ÿùJÀ99ôêù¾À;D$¶˜­á?õÚÛö¶U<@9Üùë"â?è1k©,šÏ¿‡Ç·—¹ù¿½	[]ô§Ý¿Óâž/Ö\n¿àSݦ6AGNbcu@¢B²-VLogParabolaSUMSS J195945-472519?í'@	‹€?¿ø9.—?³íÿ¶ÿ½?¿ø9.—?ìý"…³ˆ®?Á£–¹‰?¸[Òcº?Á£–¹‰?éûþÝ&rl?µ›5ru
?È‹f6Q?µ›5ru
?êžFˆ`È?¥<e'ÑŸ?ÄéåÞ|ß?¥<e'ÑŸ?í×nâ?¹~–qNªf?·AE\ºó?¹~–qNªf?àْqËä?Ñ°²a³ñ?ßôLÛh8?Ñ°²a³ñ?êtkQ)4Ï?´½€Æ Õ?Æ.R»[,Ä?´½€Æ Õ?à*è¢|}e?¸½
Xï_"?ߪ.»5?¸½
Xï_"AGN3FGL J2000.0+6509@X€Ì¿Ì3J@1ª_ÏspÀ7h¢q¯oÅÀ:¸aÏþ°u?¤âÛÊƬ@B"FY?þ!±á9u¿Ù¿Ìhù¾¿à2'U†ß¿Ú´Oñb‹ï¿Öƒ×¢¶PAGNbll@ž­‹¬q
PowerLaw1ES 1959+650?ïÿmÜ&†ý?,g¹D[Í?D€½äò¸?,g¹D[Í?ïÕÃB¬Å=?ƒžùVJëÞ?u^¾êõv?ƒžùVJëÞ?ïÆÖ¿¦ñ?'ÝÎOgw?|" Ç}?'ÝÎOgw?ïþ…ÜÎLª?'o•è>û?'¢3yÄ>©?'o•è>û?ïþÂu°Ü+?&¤MŒ¦ë?#Ø¡‰:(
?&¤MŒ¦ë?ïãàBS?®7̍÷IÚ?cƒû%9p?®7̍÷IÚ?ïèøCöò?zæÔÖüe?gìùâx?zæÔÖüe?ïùW•E?Cµåw-I5?J£è)N@?Cµåw-I5AGN3FGL J2000.1+4212@SaqýÌI@ªE`zîÀ9A›\è8cÀ;!ÛjõA`¿òöƒ—¤¡à@ÅWìÐù,@¾3Ÿi½3¿ÞšXFú ©¿ã¨ž÷k÷¿êŠ"ë"çû¿Üö§‰‹AGNbcu@mþ($xPowerLawMG4 J195957+4213?ïüŸ¼"'[?9«ÝC¬?;*K!?9«ÝC¬?ïǚjÇ@"?‡Ì"ç¯Üd?|2ʚÿÞe?‡Ì"ç¯Üd?ï˜R}‡¦?…YJ
1ª?‰ë|.zl?…YJ
1ª?ïÿ͞6"ð>ô.qI	´ù>ù1R:>ô.qI	´ù?ïôYÖW‡s?\ÕJ¬?WLS:óš?\ÕJ¬?îÒáœ?µf'Ø¥¶?¢Ñî¬JÅ?µf'Ø¥¶?î^ÒÒ["5?Ÿ?˜°á?é?ªÒÖ×0·?Ÿ?˜°á?é?ïûó58¾Z?@ëB@}ÿñ?@3+ªÜÞ?@ëB@}ÿñAGN3FGL J2000.4-2926@'Íä ¦hµÀ:ÿyŸÿhÀ9WMî \+À;jE­‰:§¿Õêú†÷ß@c²åE°@ÕúÁ;t¿é†pÞÓÇ¿æÞSèO¾¿ç«v-ƒÆÉ¿Ë1Æñ~YAGNfsrq@€Ç>aÏþ°PowerLawPMN J2000-2931?ïúežŒ¿ä?Hócúñ?Fi"õXG?Hócúñ?ï¾ù3¡ÜÎ?¢)x-êó?€A³ Ͼz?¢)x-êó?¹
?ƒiù§Ë?ŒÒ9Ãý´?ƒiù§Ë?ïû¤0vjk?2l'('µ0?Ao>þðçÿ?2l'('µ0?ïâ!D'?uhZ®Ñ?mÞëÈ7/?uhZ®Ñ?îüN'Å?¨¦¶Ôç@? ?Û8,º?¨¦¶Ôç@?îcFá»ÇA?'ýg,0¡?©Ë'æ×@í?'ýg,0¡?ï»dÜO?zþ¤KN]?=æÐç2?zþ¤KN]AGN3FGL J2001.0-1750@7ýJ€àÀ7%A` JÀ8…Þs¾=¾À;G¯e³¹¿ÙLAþcXü@¤Ð.@z+µ—Ò¿â@0œªñ¿èö‡Éëúm¿Úê"65ú–¿å"ì0•IAGNfsrq@Š±!–R½PowerLawPKS 1958-179?ïÿºßÆÖ>ý@"Ææ?H)–Ašô>ý@"Ææ?ï|jö²¾?°øðÿ0D?r¡)¨<l?°øðÿ0D?ïގû¨Ná?t:ÈÂÈX?p¸'+(£¾?t:ÈÂÈX?ïÿÃæZx®>ðIéÏ>þÂ@B1w>ðIéÏ?ïÿ–˜TÂq?
Þ ㏎?
YߐmŽ$?
Þ ㏎?îCʋ'¼?¹4I¯0?«ÃWEE¶A?¹4I¯0?ïª<tOˆ)?"µ_Íä݌?…pâÞ_…ò?"µ_Íä݌?ïÿ
D±?u ?žUoåíb?u AGN3FGL J2001.1+4352@SÄŸê³@s•À8–À7Ô¿ª¥À:k$;H«?ÓH îÀ›@T/(6ªâ?ÿŠsž³3ô¿àù ÀTnl¿à8îCȊ¿Û:K•Õ"Ç¿ßÕü#°AGNbll@›3+…¸RPowerLawMG4 J200112+4352?ëã\Ëg6?ÔÿnhF?ÀrŒÒc)?ÔÿnhF?ï·wôê^i?"äUY¢?'"À@û²?"äUY¢?煮‰Õê?œd®Í«?…ÝÁ©½…?œd®Í«?ïÿg4¨ºZ?èÆR×£Y?gcBN?èÆR×£Y?ïûYÀ:Ã?K¾D䀆š?B˜þE¶Æ?K¾D䀆š?îàP#rº¡?²eæ´Œ*?¡úýĈÒï?²eæ´Œ*?ïœþª"<T?lWô%r?ˆÀU^ðêþ?lWô%r?ïþµ'‹œð? N¾×¼A?$¦äV ®? N¾×¼AAGN3FGL J2001.8+7041@YÕÑ_ÄÖ@3õÕߛªÀ9‰´	‡h?À;""²Çì?à̈́ò\@
‹oK<ih@§`¥aÏ?ïŲFŽ¯±¿ä—¿iÉ¿Õˆ&xqi¿â:&ù$TÚAGNbll@¤Kéã½PowerLawTXS 2001+705?ïúgñg*?MZV«?F`:š˜<?MZV«?ï›òû=V*?'\Ÿ¼?‰A>håT?'\Ÿ¼?ïÁә"ç?z'Mß¿©?3tÖÔ~?z'Mß¿©?ï"}ÎÚ;?~Új¤Î}ê?›®PF$¸­?~Új¤Î}ê?ïír«n-?d^àԈ?bû•*zL?d^àԈ?íËlÞæ?·Qï|QQ?±¤ŸjÀ|?·Qï|QQ?ïoW^5ÀV?DeacM?'4 ‹>?DeacM?ëš`½@N
?©æz¡E…Q?Á–}
þÇØ?©æz¡E…QAGN3FGL J2002.7+6303@X
FŸ÷¬@0oò ClfÀ:i¨+,ÔtÀ;á|lb(ê?㙵·÷'@ý&±ÅŠ@#¿¢Â¸¿ä¡?[pz¿ìÒu³?ÀÔjÁÑv¿ÚsÜ
­XAGNbcu@¤_Æ?PowerLaw1RXS J200245.4+630226?ïÿzW›-ª?É­üâçÁ?µ.¾z?É­üâçÁ?ᄄ§~‰ž?‹ÅÔvi‡¼?€UÖ+\X}?‹ÅÔvi‡¼?ïëÙ2ò×µ?RMÀBÉÕ×?d&Í!ÅóK?RMÀBÉÕ×?ïܔmµ»
?]»¶CWT?qµÉ@ŸY+?]»¶CWT?ïþõÑâ?gäûRˆ? ¯ò3×"‡?gäûRˆ?î³¢ˆìH?©lo‡]"?¤Å×~T‡?©lo‡]"?ïÚ.á® ?túNŽÑ
'?rè pð!?túNŽÑ
'?ïŽiñqƒ?†^_˜?Œeƒª~u$?†^_˜AGN3FGL J2004.8+7003@Y¶Â!y@3téÅ+À9ò	7´À;‹ ¬Gò?°Ð®q¬x@ÏÇÓé¢?þ©€Â]2¿å÷\UÉé¡¿â§ÆZÂÄ5¿Ü¼»ŽrÊ¿ÇâzwÚAGNbll@°énÙ‡+PowerLaw1RXS J200504.0+700445?ïÿT›á?J"$UD<?Ðäò»?J"$UD<?ïֽń]?ƒƒð€r?t¡G"¹=?ƒƒð€r?ïð½pŸ‹‡?kîoòœ¹5?^…DÙðÂ?kîoòœ¹5?ïý¯Š¿¬?¹ºï-`?2ƒ¬b/:?¹ºï-`?ïþ¾Fµ{?"}›EÇÕ?$¡±°s?"}›EÇÕ?ïúBŽ3?°;á‹(p?ž`·ÁF¬?°;á‹(p?ïçU™ånÚ?s?¬ӎï?hªeõu^?s?¬ӎï?ïïr¾…Ù–?Töc×9¾?`A8-ê±?Töc×9¾AGN3FGL J2005.2+7752@['¡ Ï@6¿¤Ÿ‡dÀ8š°hÀ;~¹Ù«?ôÍJtm@Ët‡ff;@¿Ý¿ŽJÜ¿àã?˘¿ãÄÊPà\¿á©ðìçŸa¿ç¥eµ2ÒAGNbll@ûöÈ´9XPowerLawS5 2007+77?ïý¦ãs?3Àã˜<ã?2Èæ'?3Àã˜<ã?ïÌG"œ¸;?‰Ô¯«eM?yÜ5Æñv'?‰Ô¯«eM?ï¾1¨]p?~Ù²	Î?€s•î{2¥?~Ù²	Î?ïàæ"PS¢?P†kïX)?o{óµÂ?P†kïX)?ïûX±¥‡—?Cà¼Âۀì?B9÷J?Cà¼Âۀì?ï%*¢H[?¦¿€Û g?›Z«¸¤""?¦¿€Û g?îÞ/¡¿i?›É¯áÚ{?¢áu¹0?›É¯áÚ{?ﶓÊoä?uLttB[?'[
fø¶û?uLttB[AGN3FGL J2006.0-2311@2ø÷àvͽÀ:-Z@¾61À9/?ÐÐgŒÀ;}|Ùor?îŽ"é+@hö'äöd@ö?ŒÝÉ¿áØp+â¿çrDoè脿ë™IÙõL¿æúÓÓ§1ˆAGNfsrq@ë$Ý/PowerLawTXS 2002-233?ïÿ-&v-Ñ?ß63
Ý{?[1¾6܉?ß63
Ý{?ï¥Ô±%Z
?"¸1pv›Ï?†ŠÓºk?"¸1pv›Ï?ïso IK£?Œ§
Á ֖?''ûýõ‹?Œ§
Á ֖?ïÑÖþî°?X\âv²¯Ú?w€…kx@?X\âv²¯Ú?ïþCt@f?.Þ=7R•?+È¿­eݯ?.Þ=7R•?íê2ãý?¾î÷™ÿðç?°®k–=c?¾î÷™ÿðç?ïvEµŽ?"jã­÷»?œ17Qó47?"jã­÷»?ï liC?‹ûYö…G?œ«òt—¥¥?‹ûYö…GAGN3FGL J2007.3+6605@XÏè?ïÚ@1n´_î}!À9€ú:þÀ;'-±2ã?ÚQð"
yÌ@VÆwÉS@·ò ¿ãn×Ѹ™å¿ê°Ïb «¿å0Ì6àøå¿ïþ•2ñ]ÀAGNfsrq@'AKûµtPowerLawTXS 2007+659?ïà¹t'ˆ?­¿Y"îO"?oF‹?¼Àÿ?­¿Y"îO"?ï¸mø+h?Š9ð-þU?äæÝö?Š9ð-þU?ï§G`Ös?|á'êv?†>..©› ?|á'êv?ï~®N;w?kò,v¹Ak?*=™¨-?kò,v¹Ak?ïù¼\űX?Xü¶›ô?I‹çñz@?Xü¶›ô?îWûµª?²™–ÉU€?ªŽ.pD¥e?²™–ÉU€?ï†`·zÖ
?‹OpSð°?ŽgÒ+™Qn?‹OpSð°?ë⩘jD—?¥ÓR%{_?ÀuYžVí£?¥ÓR%{_AGN3FGL J2007.7-7728@sË/ŸËÀ>Œ6`]'À9sÔöfú
À;›wï$æi¿°áõ"x'@ÿÀ+©§@výòÿf¿èz'V?ñ¿äòu¥Õ¿é¥þÓôÎ
¿ïÿ?9!AGNbcu@}›š¿4PowerLawPKS 2000-776?ïûŠãq*?D—Ï;âˆ?AÔrÉ ?D—Ï;âˆ?ïÒ*ÎFØ?†_^#:±q?v꘾?†_^#:±q?ïC@ûŒ˜?Š¹(Êps?—Ÿ7×÷g?Š¹(Êps?ïôxz
??ZgÛSžÉ?W
|ã,ï??ZgÛSžÉ?ïû*µ­˜Ì?J®´4ii?CU(Ö)ï?J®´4ii?ïLTo¡"?¤€_MýÀ´?–ur

¼?¤€_MýÀ´?î¹Kà>?ž,í&'¤?¤kAûú—?ž,í&'¤?üÍñ?|r£?¸Üý\ç¬?|r£AGN3FGL J2007.8-4429@v6Ê?‰'ËÀ?ÕŸÕó½À9ŽTEÒr(À;­†Q¾8µ?ÈE'² ¤@F´šQ@¿œÿªšž¿ã>w"k4¿æä,J
æ
¿ë:ï.˜ç¿ÙÁ6ÓÉÆAGNnlsy1@†( [ÀPowerLawPKS 2004-447?ïÿBÇ$í?1†šjáÛ?ס6Ú±?1†šjáÛ?ïÉ៲?Š¨2Uìp?{w,·b?Š¨2Uìp?ï´Ùr—'?€m4;¾îx?'ɺó€E®?€m4;¾îx?ïñŠ\mqÑ?HÄÞÓÒ?\ëF´i.?HÄÞÓÒ?ïý%ÿ‡ÎÛ?>lõ&vo=?6Ð^"jó?>lõ&vo=?î¸çNr¹?µ¼DÎTûõ?¤q‹ބk?µ¼DÎTûõ?ï_ÿi#§q?~¯G%ºl?"âjIÉ?~¯G%ºl?ï.Õ\'%Î??x›/6s?š%Tvš~+??x›/6sAGN3FGL J2009.3-4849@uæ
 '§À@LZ&–mÀ7ӊë€ìúÀ:©³%[Ú¿íükl@@€¦Kٝ@?ü_ãìŸP¿Øfû"¿h¿ÛvÞX»X¿Ö2ä%Pi¿×-	þ±vZAGNBLL@¡þ‰7KƨPowerLawPKS 2005-489?ïÿPQ?ý`? JZî±½?õÜìÎï? JZî±½?ïÆB~¢Þ?•ن0À™?|ÞÀÁƒôé?•ن0À™?ïs£½×2ú?'ùv$Ô³'?'‹ˆJA
Å?'ùv$Ô³'?ïÿï[dw>×<"éèã>à¤|®dO>×<"éèã?ïþ‰­_Á~?*Kl ?'e)Bd‡
?*Kl ?îæu!{a?·â@È	S?¡ž²3Ìê?·â@È	S?ïª^ҍó?ûs°$@>?…hKYIç8?ûs°$@>?ïÿ¢3_í•?´['´Ü?s+¯%½~?´['´ÜAGN3FGL J2010.3+7228@ZVhÍJ¡@4$WÀ±5˜À9`¬é·À;Øwûº ?ö" =͕õ@Š•DË6@£3ø€ñ¿áí¬¼ó!1¿ä+ÚûIóû¿å{ÿUò6$¿ëêHeì»AGNbll@†}2€ñ,(LogParabola4C +72.28?囹îjE?ˆuuU #)?†yzšÂ?ˆuuU #)?æä•cÝ}¨?Ç¡—r€ƒ§?Ò6Õ8E±?Ç¡—r€ƒ§?ìRqèXL%?©¡€z±‰?½lp½=žØ?©¡€z±‰?æm)x–·	?¡&°åWá}?Ó%­ґï?¡&°åWá}?ì"§)¥ø?¾>`ìKe?¾êƲ×XA?¾>`ìKe?Ó´ ©‹Ý¢?Ëa›¬ÕqÈ?æ%¯«:/?Ëa›¬ÕqÈ?æIdÑ"?´ä,;9•b?Óm6]Î×?´ä,;9•b?ÎÁ(|©|n?¦FæÞ	ÏÑ?èOµàÕ ä?¦FæÞ	ÏÑMIXED3FGL J2012.0+4629@T"GŸÑÁÿ@ƒ32ÚÀ8PݝÕh}À;<äŒÜóÀ¿Ï+šã@Œ=AT@@Ü= ŸrL¿ä©‰[¿ã÷Z4,¿Ö?H=9$¿ã0I'f2uAGNbll@›®TɅðPowerLaw7C 2010+4619?ïÿ¡>Bl?ƜÀÑL"?¼{˜M?ƜÀÑL"?ïÖÍNä?{Þ
£¨˜?t™x:¼ýì?{Þ
£¨˜?ïêç8õ6?cs'á.¡?eòÄ9@?cs'á.¡?ïÿÿ-‹î$>®Üq"¯5Z>šPPDå£;>®Üq"¯5Z?ïþùUýôž?áˆ^¦5á? jžŠù9?áˆ^¦5á?îù£l¸?­÷0Êå? eÏÄâ‰?­÷0Êå?ïçê˜mRF?r¸'ËKß?hgx±¨?r¸'ËKß?ïÿòß¹—>ã")É-KQ>Ú@fzfO>ã")É-KQAGN3FGL J2012.1-1643@:=ÓÀíÀ9)?O¡(À9´a¼æÀ;°}À?`?û+çpÌ@¦5þ¿Ž @æsžg}¿Ò&ÞJ<}ù¿ì—ÁÜȇ2¿ïôƘw§ú¿Ùú39Š²˜AGNbll@€¤?åÉLogParabolaPMN J2012-1646?ïÌýœÅÀ?"37êñÞ§?yüMÉë©?"37êñÞ§?æÐ#y+åâ?Ñ}"rÒÊ,?Ò_¹
¨4<?Ñ}"rÒÊ,?éÊ
˜þ?³VÍëP‰?˔××±œ	?³VÍëP‰?êù§Râ?®bçã ñ?Äb´wÍ?®bçã ñ?ïôÏö"¹?g~ºH¥[%?V`Ô±½9?g~ºH¥[%?ÓQQÈ/ë;?Ò ù;ÑÎ?æWWè
b?Ò ù;ÑÎ?ë̬Û.©?°Ì¿Àš›j?ìÍL"E[?°Ì¿Àš›j?ÜÄwY¹ëÛ?É*%‰b¥ù?áÄS#
?É*%‰b¥ùMIXED3FGL J2014.3-0047@Dýžà*w£À2ºÜ fèÀ9wU4åºÚÀ;Fù	q?Ø&‰åz `@5dЏ$ ?ýP!?Àµ?ç]G¦²±Ä¿áÙÅ(yØ¿Óè}†­G¿â'²Íƒg9AGNbll@®Ä`[À7PowerLawPMN J2014-0047?ïýò+¬O?,ނo0}Ò?0n ïáág?,ނo0}Ò?ïh"új·%?§È€±Èê?'퀫Éã]?§È€±Èê?ïßã&&Á?k•
Ñu?p€i!?k•
Ñu?ïñ>ß8à?A5LÉ`?]'Aëµ(Â?A5LÉ`?ïû… Î?A¿'á`?AëçêÉ5"?A¿'á`?í\°çáG¥?½è $Ö­?µxÃ"Q?½è $Ö­?¦öøwÿ?€l+e.?€Â7;6R?€l+e.?ïÓ;$T"M?f(-¢ å÷?vbmâq{?f(-¢ å÷AGN3FGL J2014.4+3606@Rw	ÎÒa?éƒ9õÐôÀ8íaö•À:i"ïQ0?õ'2T»ï@xq5¢NI@0~ÀzY
¿à	Ç^ÎÂp¿ã­¬`›¡1¿ë>H:+tù¿é&¯â[TeOTHERspp@šs•fÏAòPowerLaw?±}Dd×!?½¼ÎR
?íÐW~A#Œ?½¼ÎR
?ÁÓ6.¡d?ÅA¬p"pC?ë¹2tW§?ÅA¬p"pC?ãŽL[DÁ?´cçâÑÁ?ØãgIv|Å?´cçâÑÁ?Õù¥›¹.?¯àšS
»†?å-2#yé?¯àšS
»†?e4Tn_å´?ve—½]?ïêË«Ãz?ve—½]?œÀÞ¤]p?³oS:Ë6?ïù!ϼ?³oS:Ë6?ÇË 6¸?´Å^y2?ê
ò~ÑÜ?´Å^y2?¥¸øµ'1?•'håË
%?î¤pt~¤m?•'håË
%MIXED3FGL J2014.5+0648@Hw V·À.€LÁzÀ9o>À;T' ¦Ô¿Ú}ôÌ_‰@fSvt¦p?þ¤®àþˆ?çW­ËÕ¬¿èU‰%û^¨¿ÓïKº
ß¿ÙvŠq™±~AGNbcu@±6NzáHPowerLawNVSS J201431+064849?ïýîW6?5q 	ºç?3ðŒŒÕ?5q 	ºç?!]j6?œÂSå"Ã?Žw¨¥r?œÂSå"Ã?ïÑHãÚÁ"?rµR…ô­?w[Ž®d?rµR…ô­?ïý† J? âÜÏA?3ÎÿZZ±? âÜÏA?ïøÈsvÅ.?J`|å8üú?LÞ1ËOö?J`|å8üú?í³©eÈ€?»çOÛ?²b´ÑQ˜ƒ?»çOÛ?ï¯ßþF±.?ƒcÍÇØøþ?"e"?ƒcÍÇØøþ?ïð#¥»TÄ?U4´L@?_¸´üÉW3?U4´L@AGN3FGL J2014.9+1623@L®¡@W%À$;ÿwDÀ9Õ(X䝤À;qhµËÿG?ºâÌÆö&Á@%2?@G]Ÿmn¿å‡'(Ap@¿æQ(óØï	¿äýt½1­¿Õ¬s¦jãNAGNbcu@'fÖ"uPowerLaw4C +16.67?ïüf!5ôr?D»^Þ5r?<Îõß g?D»^Þ5r?ï€ÅÜ:?¤Ç&^}R«?ùŽ¸Ut?¤Ç&^}R«?ïÇJ5	ª?vn–ѵ4@?|Zånè?vn–ѵ4@?ï÷E˜h0?8hS•"?QuàâmoÝ?8hS•"?ïâÿ7
â?v¸ r4?mÿ¬fo?v¸ r4?íAµÑwp>?ÀIUÐRN"?µòQtD~?ÀIUÐRN"?îùžtþ7\?˜S'p§Õ>? f³Œ&B?˜S'p§Õ>?ï¬Ò­¿e?vii¼ac«?"ËTµ`Šß?vii¼ac«AGN3FGL J2015.2-0138@D§:¶~­À3XhÌÀ9%¹˜<¢HÀ;^||R`ö?ì8_Œ¤àí@
Í,݃©B@7* ís?±F(mÝS-¿åð"Ò.­à¿ã‹ü]¼§C¿åRÜN[>AGNbll@˜æ€hۋ¬PowerLawPKS 2012-017?ïwß`?•'§WµX?'ÅËÊÆ?•'§WµX?ëKÙ¿›Ù?Ã3¢­5ô?ÃöЙ›?Ã3¢­5ô?îÊqm"À?–¡WýG?£Xé1N¯û?–¡WýG?ëN÷ì$Õ?œiYkôHP?ÂÄ Oo˜®?œiYkôHP?íçÐCyÒT?´u$=l?°Á}å{Gß?´u$=l?×zÓñ.Uÿ?φ†p¶»,?äB–hÕ?φ†p¶»,?ë:ADmî?±»%^Îv?çúîHH?±»%^Îv?و=@¨;É?´T6Îá3"?ã;á_«â?´T6Îá3"MIXED3FGL J2015.6+3709@R·_ßÏ?òø
€CRÀ7Ïng¼¨À:+l¤nò?ÿµðÓ×@rõJð>@@îݘͿáÞ³&¿åÂóýé$q¿çxýP/¿è¤ï‰ÌXDAGNFSRQ@—ÉÃä%®æLogParabolaMG2 J201534+3710?ï?äõ±ê?²Âø{êÕ?˜a`!º?²Âø{êÕ?ï%}øÿ/Ë?²…§ièE?›P@è±…?²…§ièE?è±m?µnώŖ}?Î¥;ŽKˆ?µnώŖ}?ï_s¦j?z¾º1áñÄ?"ў£¼?z¾º1áñÄ?èÇè£Ô?Æ´€»&\5?Ìã¿ô]p°?Æ´€»&\5?ì›iFÐ?ƅIëÜ\?»$³"•É€?ƅIëÜ\?èuUŽõ?µªŒE?ÍÂ*©Ä+‹?µªŒE?îùŠ\(¹¡?"È­&•ö4? gZ;¼—ì?"È­&•ö4AGN3FGL J2016.4-0905@A+©Ÿ¡—À6úã Ì(bÀ8ࢻž§À;Bqÿ÷œ"¿Û}ˆ¯šœ@šÍ¥å­C?ÿÀìÿÈ!¿Ý(§¶_D¿ßÙ.ÁÌk¿àFbuž›?¿Ûj?ZD*cAGNbll@ 3•%F
¦PowerLawPMN J2016-0903?ïÿ¢½ã-•?Ž	¤so?P‹4xD'?Ž	¤so?ïšë'M?š³ÐÎûUj?‰|úzИÄ?š³ÐÎûUj?ï፨ìë?nP¹y?nrW"3+0?nP¹y?ïþàZÉ$L?û"Gª?!úS­€ÐØ?û"Gª?ïÿ
‰!ô"?!qYY›N?NàÛ¥Ê?!qYY›N?îPŠ^4¶
?¸!H½?ª÷Z†6?¸!H½?ïÚ
68:?uÎj"j?rùdÒùž?uÎj"j?ï÷Ð[çK?FšdtJC›?Pà_)ôÙ¦?FšdtJC›AGN3FGL J2017.3+0602@HOt cLÖÀ0:?–îÄÀ8"úgðÀ;×@Än@ƒ–ÿ‹eú@
S
ã2ê¹?ö'ª%Øם¿Æ‰Wu:rJ¿Ê£ö¿º¿Ü÷ßFïJ¿ìÁÄÜq
<PSRPSR@š.ºáG®PLExpCutoffPSR J2017+0603?'˜Íµ¸°¡?,ˆæ¯bÇp?ïþ†s!4Ù?,ˆæ¯bÇp?¤ãj¿ƒ¼w?Á Sùb".?î±ÉSúÉ?Á Sùb".?ªùÖ©Ç–?Ÿ´Xâš>…?îPb•:S'?Ÿ´Xâš>…?y#ré$£?b‰TùȽ?ï͹W3?b‰TùȽ?@HdÖjñ–?6Ælª²ús?ïûíæð0÷?6Ælª²ús?…ЈÅÁ(?¤Ÿ*òÚÃÿ?ï«ø¾$K?¤Ÿ*òÚÃÿ?¨ÆÊÀˆ9Ù?£2Ó)?îs"SÀ'£?£2Ó)?Q,ø{8Dê?FÎöXxM2?ï÷i"¼5?FÎöXxM2PSR3FGL J2017.6-4110@vz4¿ÍhÀ@À?öÀ:få2õÒÀ;ÉdÞב¿å	 Å>ÛT@
Lº–@FônJ6¿ÛýxU¿ìæRµöп´U¶ÀÆÚ¿Ïš¼ÀvAGNbcu@¢fšÔ,=PowerLaw1RXS J201731.2-411452?ïÿ¯æÀœp?wËf¼?PAOé?wËf¼?ïÏÅB>éË?ŒI#¸Öpœ?x^èÊ*š?ŒI#¸Öpœ?ïË
©ù?y¸¾~Ԓ?zxûY€?y¸¾~Ԓ?ïÿycTt]?¨hŸ‡?ӎk?¨hŸ‡?ïÿ¯ÃQ£â?	"X,?‰?7>ª*?	"X,?‰?ï+ÿ(Oæƒ?«ìÏºj?š€ùrˎ?«ìÏºj?︈‹îúä?I.y
}¯?ÝÝٍ?I.y
}¯?ïüvžX#?3ã
åô@ì?<OÓ#<hç?3ã
åô@ìAGN3FGL J2017.6-1616@;F'À9@"À:7{ßto>À9J
'/ï²À;rÁ3;–¯?ðºÌ1qg @Çö‰^¸ó@ц B« ¿ÊnЖ
¦¿áÔÇq\þM¿×'r%-ÙO¿î.
)y¡PSRpsr@šØiÇy¦µPowerLawPSR J2017-16?å—V¾}©¤?Ë$3n:à?ÔÑRƒ¬¸?Ë$3n:à?è«>¶ZUÈ?Æà5CrŠP?ÍS&–¨à?Æà5CrŠP?æ ]¯¢^S?²='†b¬´?Ó¿D »CZ?²='†b¬´?è'3…"?¤Þš/@µ?Í÷3ïé¶?¤Þš/@µ?Ö2Eç.½?Ê,²™Å¹?äöfÝh¢?Ê,²™Å¹?ÛàÁ<£?ÐñÛ5VŠ7?âŸ?uá¯?ÐñÛ5VŠ7?Ù¨Î̒{~?¿'¬âÃü?ã+˜™¶ÂA?¿'¬âÃü?ÙÎm+?ºqiº-ã¾?ã}˜ñöIj?ºqiº-ã¾MIXED3FGL J2018.5+3851@S%öà1-Ÿ?úžÂÊ £À8­°"—©ÕÀ:'õ}Åþ?éfÛ+_T@â»Z^›A@Ô6€šš ?ï·¸ˆ¿æø…cF¿ç{g;§¿×}–³é°AGNbcu@*¦€IRPowerLawTXS 2016+386?ï(ÿ»a•q?¯Bìø+(?šà—<íÓ?¯Bìø+(?ïB5yßj?¢]•ÿªF?—¹Pľô?¢]•ÿªF?ëH©>þ?®¬ó§L͞?Âß¡[¢?®¬ó§L͞?ïû ¿Š'?"Ž'$kta? ›ßw§à?"Ž'$kta?æüå|N¸¨?Ê¡Aƒ­ôð?Ò5bŽ¯?Ê¡Aƒ­ôð?ê̯° ?ÇuœpŽˆ?ÄυC¡?€?ÇuœpŽˆ?åJm³¦yì?¹ô@î¬µ?Õk$˜³)?¹ô@î¬µ?ê'<ã,¬ÿ?µö	±)8?Å·sML?µö	±)8AGN3FGL J2021.1+3651@RÎè_ÐJ0?¼éóŸÛŽBÀ5hÀwSôtÀ9Þè¬&d@ŒN¸@ý{|@ÛnÚ~;D¿ÕT.wÙø§¿á"~ièQ
¿æ¤7HÛTê¿íCÜq8/$PSRPSR@Š3è>BZîPLExpCutoffPSR J2021+3651?&}~ºw?'üUf>]?ïþ˜/ûßú?'üUf>]?¥ÅµSÏÙô?ÃÇuÜj?ª™Ç?ÃÇuÜj?p1æLe·?~›–…'~?ïßÜCåT?~›–…'~?êR¡"D>ý7G>ÖŒ?ïÿ¨V˾°>ý7G>ÖŒ?-©-$?"Ž
骥¿?ïþ%mUvˆ?"Ž
骥¿?‡QÀ¶Ù¿?¨¸º1ä?ý/¹?¨¸º1ä?vIteÀj?jÍ¿Ø÷k?ïÓmÕ	v?jÍ¿Ø÷k>àí¢'\Ï>äW¶™â9?ïÿïpT•>äW¶™â9PSR3FGL J2021.5+4026@SŽÔ2Tç@ªJ_ʕæÀ4Øï;Œž	À9҇'§
ö@K§ÍäÏÎ@>=@§:@¨[—ÖK¿Ók›
På:¿â*›Ö¤¿ç­»I–¾¿î9ïxPý&PSRPSR@"zn—OßPLExpCutoffLAT PSR J2021+4026?ÝheœÖª?Öµe
\?áK÷M1"«?Öµe
\?¢€?
ÙÅ?½"ÕI?î×üåç?½"ÕI?ВKâñ?³Sb½¢Rõ?ç¶Úx¸?³Sb½¢Rõ?#Ά\‰?s`]¥¨4?ïþÃÓlŠ?s`]¥¨4?Öà jr~f?Ñ&f²¢»=?äžoÊÆÀÍ?Ñ&f²¢»=?‰ÒN«"‰¯?©+8°#2…?Åô?©+8°#2…?Þóîô¯Ú?Æ"Ñë^w?à†ü¨?Æ"Ñë^w?|B!pvE?,êÄ>2Ý?ïÿÕd1?,êÄ>2ÝPSR3FGL J2021.9+0630@HÐu@ýAÀ0ÅM¿¦sÀ9ªwhiÏÀ;m
[£"Å¿û»T­~«@
5#·j:@s\ <`ƒ¿àJ"+y3¿à`™. 
¿á‰ûcZ¿èø°1ze;AGNbll@¢`J=p£×PowerLaw87GB 201926.8+061922?ïð
҄$p?dª›dÁëÞ?_äZÖºà/?dª›dÁëÞ?ïœfa?›Ç‡šfé±?ˆæxÝpåÅ?›Ç‡šfé±?ïÿ2-WZ?"û)ž¸Q?Œ€3j[U¡?"û)ž¸Q?ïÿ°	¦$ ?%Aåc!³?ýŒ]¬
"?%Aåc!³?ï@¢	T½r?Ÿp²ç뮇?—ë¾Ú»Ç?Ÿp²ç뮇?ípD/H±¹?À0ñ7‡´?´}ބp—·?À0ñ7‡´?í¸"¯
¹?¤Þð8T?²?Kccy7?¤Þð8T?ï÷kʆÿí?QP¿ùfF?Q(j˄‡?QP¿ùfFAGN3FGL J2022.2+3840@S6¸!ï?îÍÁ¿Ü&À7û_)[CÀ:G$ãW²@Óï` ~»@
e•ÙE¬@xH-Á.^¿ÝÐdÜÎw¿è‰œ*Œñ¿ë.P«>¡¿ïÿ†ÈÜ}DOTHERspp@"¥®æ1ùLogParabola
?kúYi}?';W>â0:?ï䦻ž°?';W>â0:?¢É`"­[?½ÕÙ:ï?>?îÓnyÛ8J?½ÕÙ:ï?>?ÊFÝiÓq?± QÌSê´?énH¥‹?d?± QÌSê´?'TÌ¢
é?i1éÊy?ﶬͱË?i1éÊy?…7[á
ˆ?›[{=ó\'?ï«#ö{Ê?›[{=ó\'?‡ºñº	T&?¨-‡«?ï¡8ààð?¨-‡«?Æ´qÓGg?³Ó³…xÜR?êRã‹;n&?³Ó³…xÜR?M5J虎??×8<bˆÊ?ïø²­"È??×8<bˆÊPSR3FGL J2022.2-4515@v.F_•'ÍÀA:2 f<uÀ9°Ö?<VÀ;»>©ˆúæ?Õjˆ6<I@˜þi'@ÄAÿÿª¿áq—->㧿åõ7¿ßÔf¿æ‹"\!¿¿å³N÷^òAGNbll@‰ü`,'PowerLawPMN J2022-4513?ïþzd?6½‹yG‡—?/&׬©w?6½‹yG‡—?ï¶ÌH 2Ù?š3³Ný?'Líù«¿?š3³Ný?ï®ÂKП?mCÒڄ?"|OwZ¬(?mCÒڄ?ï§Ê·sÊ'?g!†Ë©;Ä?†
ROH?g!†Ë©;Ä?ïèX_xÇ£?v—0gÂ?g§ hûÍ?v—0gÂ?íwo!9ÐJ?½ø…7aì?´D†õU–°?½ø…7aì?î}BáQC?¡%™Àуû?¨+ÑêäÑ?¡%™Àуû?ìÅåŽú?¥j˜D|?¿9Ðӏ0?¥j˜D|AGN3FGL J2022.5+7612@[Sc€ß@5#ô™=SÀ8߃'gMÀ;€Å¤º_¿¸AÅ(£@Ëbôkø!@ÍÄÀcÝË¿æ|V'0¿äs ¾¦ïC¿äYž¿ʵ¿æX
6n|AGNbll@Œ[ŠqÞi­PowerLawS5 2023+760?ïýèÔk?*~z•NÔÅ?0¿>nUs?*~z•NÔÅ?ïØ^fùÅe?€?*qÊq?sÐ̏{åª?€?*qÊq?ïâb*—ƒ??oV:1ô«£?mÕr©?oV:1ô«£?ïæc µJ?S"…	Êà?iœñrˆ…Ž?S"…	Êà?ïø=µ?Pc!ÍW#º?OªîLè?Pc!ÍW#º?îÿ¿´ !?°h}¸? ¿©äð?°h}¸?ïOÆÊVr?'.e\êÖg?–*$Ͳ?'.e\êÖg?î½é/ô?–#ô"'@?¤!o
€µ¾?–#ô"'@AGN3FGL J2023.2+3154@QÙÜßÔçNÀ']ßYAeÀ9nwºKÀÉÀ;6jö ?ëÐ^_0çÿ@ çiõ@'x z´Q?ížf5F¼[¿ ;'Z鎿ãZsæŠA¿áIÑJ¾rËAGNbcu@©õ­quŽPowerLaw4C +31.56?ïöïç¶?R±­L¯Ð?R àA ó?R±­L¯Ð?ïÀNƒå?±¨cêhÈ?œgöD¦‰R?±¨cêhÈ?ï¢f͝	ï?…&a»P?‡fL£X*?…&a»P?ïFiŒ>Dè?{曣´£?—2Κþ?{曣´£?ïá–iÓ6?ni–
‡²*?ni–b}±°?ni–
‡²*?ë èÝ"?ÇmKA
Ñ?Á|\‹µð?ÇmKA
Ñ?îa¹x~? =µø>?©äo½#? =µø>?í7'
÷!W?¤_LÁ¤¥'?¶Cw©þÃI?¤_LÁ¤¥'AGN3FGL J2023.6-1139@@O¢ŸÒ˜¿À9®â_ܪÀ9'`uÖFÀ;T3—Ac?ò´bÞ©ª@µL¨z2?ÿV´öí?¦,EG ¿­¿ÚZ"|<ø•¿ÙÆ»®ÊáÄ¿çz8B'ŸûAGNfsrq@Ÿ»P|"µÝPowerLawPMN J2023-1140?ïhhÇi¶}?¡#'ýi?'òçÉ0`?¡#'ýi?íQ\ä‡~?¸P(@`Ï@?µuÝ{ن?¸P(@`Ï@?ï9¯p'Ý?"k ޒŠ?žøÊ"ªc?"k ޒŠ?ì€sl֏f?'ŽG7k?»üd™K"Ò?'ŽG7k?ì.«…e–C?¾Ecï5#ñ?¾Š£ÔÓMè?¾Ecï5#ñ?奐8Øõ¶?ʱY^–
s?ԴߎN"?ʱY^–
s?é»+Ð|"?·@›"F+?ÉP¿¶
ï?·@›"F+?å»°ºië#?°97ÌMŠ?Ԉž‹,)»?°97ÌMŠAGN3FGL J2024.4-0848@AƔÿÖåUÀ8££Àd¾À9¹Í°!›[À;[Ö¥"¢à¿Ð&m2ï|¶@—pÛà;?û=ßÿ¯x(?ìñÐÖi%¿Þßo1CD¿Ù^ß§¿È°ÂHB®AGNbcu@¸î_ö"PowerLaw1RXS J202428.9-084810?ïþ±$5ûv? ˆé'T…œ?$í½+âÃ? ˆé'T…œ?ï"ýD'»õ?§xâ 
ÜY?ŽÀ®ò¡f¥?§xâ 
ÜY?ïÚö¼ñs±?qúë!+]Ï?r"¡tWi?qúë!+]Ï?ïÿ9öP?—#ÿ¼§Ó?Ýçˆ	œ?—#ÿ¼§Ó?ïý¦åvV??©3?7jÉž±??©3?î_Ljp|?µ(nÆ´‹?ªØTß8?µ(nÆ´‹?ïÀ½Ä`"?~íYg€éß?¡¹Oʟ?~íYg€éß?ïüzƒ$Ç?4"·-ÆS§?<+颵ü}?4"·-ÆS§AGN3FGL J2024.4-3254@#>óà¿À@n¦`QyoÀ9<ÚvÙ{1À;@#¾†À°×º'‹Ù@å5O?b@OêÀ'ÍÏ¿éÄ:ê.)¿çØ
Ù¤¿âÉ	7¥ø¿ï¢3äÔAGNfsrq@tÈá|ÚQPowerLawPKS 2021-330?ïüÛÔõ?<åIdÏ	?9'÷>Î}Þ?<åIdÏ	?ïÔÒ¿óÜ?éÿ:K?u– }$ú$?éÿ:K?ïN`þW?Ù`ø̵?–3à/¿±?Ù`ø̵?ïÿÿ*SKé>§ä[»Úâ>š¶üáÀZ>§ä[»Úâ?ïþgÔGû?-G1Ë_i?)'·âÃh?-G1Ë_i?ï\—(-Ï$?¢,{è~?"m%S}?¢,{è~?ï]E­€£¡?'n‹S#Ì5?"WJISï?'n‹S#Ì5?ïÿërªAˆ>í%SïB`>ä'ËGˆî>í%SïB`AGN3FGL J2025.2+3340@RF–àU­ÀOÖOÀ7é£?4É5À:^zb?øÐ{ùF@…'Ԇª@ئ²†Ði¿â±Àç]¿¿éŠù‡"³¿æ"@¢Ã ¿íÍVœ2¿àAGNbcu@"i—
=p¤LogParabolaB2 2023+33?îÄ/õ Ö?¦üûRl˜?£½«:o¬?¦üûRl˜?ïTõ©vÄ?­è8ŽúN?•aJÒôõ"?­è8ŽúN?è`k†r½?±Ä'sc
¼?Î~Qæ7é?±Ä'sc
¼?ïyS¾÷±?qiSâ"?ÕˆèŸÙ?qiSâ"?îð3YHÇ?®Úå´J+?¯@üζö'?®Úå´J+?ìÐ3óç1Â?ÃÆtnÿ­?¹~`a4er?ÃÆtnÿ­?é'±'?²ÌH)7Òl?É·ëÝ;ãd?²ÌH)7Òl?îáæúËb¿?'U·ì:Ý?¡áV¹p?'U·ì:ÝAGN3FGL J2025.6-0736@Br® 9[kÀ8d:ঞeÀ7Wm¯0ÔÀ:æX"»@ܺ«@7ï<ä7@xãPÇÄ¿ßRáù§u¿å¥¨×¶F	¿æä¦É¿ëÁuuoe5AGNfsrq@Ðå`A‰LogParabolaPKS 2023-07?ïèç(SíN?aƒèjªžE?g×¥3y×?aƒèjªžE?ï}n^ò¤?¥ö@ˆ+?R4%,§?¥ö@ˆ+?éÊÆ=D6Ä?°•ˆ')J·?ÈÔç
ï$ï?°•ˆ')J·?ïúã®ïå?4òÝÙÜ"?DqE»˜"?4òÝÙÜ"?ïvŸ Âg?ã2â!ë?',étá?ã2â!ë?î	½kZìá?½4Vøùë-?¯d)Fá•ü?½4Vøùë-?ë¤ãoüg?¬ŽâØéö?Áo"r@c?¬ŽâØéö?ïüŽ¸âV™?9cbAûÔ?;Š9Žì¡?9cbAûÔAGN3FGL J2026.3+7644@[z°<«'@54·¿õMõÀ:"TÊÀ;ÐóöÝA¿ò²cЦ÷@·…:<ý?ým8ÎAl?ì™Nw©§%¿½†"¯¿ÜÞj)К¿éäÁªÒ'AGNbcu@¿¿ß;dZPowerLaw1RXS J202633.4+764432?ïä²uøC?l€Ï5Y]?kM‰ÖBc?l€Ï5Y]?ïÝ
a3îç?|Bnjü~?qyOXJm?|Bnjü~?íÛëÄðƍ?¥1A€"Ü?± ¡ØØ?¥1A€"Ü?ïýŠK.¨?&ŽÀÎ@7?3¯óÁ¨LÅ?&ŽÀÎ@7?ï§ZÁŽø?ˆ¿™sßÚ?†9iYëÔ?ˆ¿™sßÚ?îŶâ7 ?¶XRþœÖú?£¤žQ܎?¶XRþœÖú?ì¢ՍT?®±…äÿö?ºï!S•[û?®±…äÿö?ï×öT8D?r8ôº
ï¸?tÖÚ1q?r8ôº
ï¸AGN3FGL J2028.3+3332@RW€dÀ	¾ÀD©'À7xrϏÀ:pŠ)º
­@VVù¶æ@}$îÌÑÕ?ü£_9M¿²²U/åÔc¿Ú³íéä¿çýuûÉ~¿î:öå¥PSRPSR@"ð&šÔ,=PLExpCutoffLAT PSR J2028+3332?3û°¤¯}:?/—\ñÿ?ïý€‰Û¿?/—\ñÿ?£;ÛҒù0?¾lɨ'?i?îÌBB'=?¾lɨ'?i?*ý³–è?«zè_˜?ï‹UÿÄyu?«zè_˜?}i™¢W-?drí¤…öB?ïÅ,Ìß
¹?drí¤…öB?7"׶p7?1áõŽ:J·?ïý
dö'?1áõŽ:J·?ƒIAÝYÄ?¦ÏØÙÝ?ï²Úø€ý
?¦ÏØÙÝ?tÝD_D¥?o(8–éøÂ?ï×òE_ä?o(8–éøÂ?Q»à®
"r?D^Ë\a§—?ï÷"Á¶f?D^Ë\a§—PSR3FGL J2029.4+4923@U˜WŸúë@Z
@JÈÑÀ8rÞN«_À:úō=jÅ?óÁz´&8@o*s*©@I:ÀETô¿â½'ö{-.¿àb|>Œ¿égóI8X6¿ì
GÃ^vAGNbll@ŠpVOv`PowerLawMG4 J202932+4925?ï]©ž?Ÿ–¡}ÏÊ¿?"_êÔÓ4#?Ÿ–¡}ÏÊ¿?ïZK˅yý?¥"†*ïi?"¶†PÀb?¥"†*ïi?ë0,ß~x?©ÿ"~µd<?Ã?§L'!?©ÿ"~µd<?ï`ùXà±?v»êf
¬ô?àÓ,ï?v»êf
¬ô?ìÍӃ'ð½?¸þ\ n?¹'cåä"?¸þ\ n?íK§(«ùK?ÁL:‡ ¬Y?µ¢Æº2B'?ÁL:‡ ¬Y?èõÀ$Yñ?°cZ‡ÿËú?Ì(ÿn›Ð<?°cZ‡ÿËú?ì6ö©Àd?¥®Ñ(Å?¾HJ±ÿìà?¥®Ñ(ÅAGN3FGL J2030.0+3642@S~ +ïr¿öçÇ¿Ç«¦À7΋ýϤÀ:ž;aÕÝî@øByw:I@ړ‰à?ø»B¶³Ûº?³ðïèkõÙ¿Ø_ÄŠŠ¿å«Lh¨#å¿î"¨FNPSRPSR@˜
Þi­BÄPLExpCutoffPSR J2030+3641?mo7Ö¼?®E.ðCς?ïâÈ('	?®E.ðCς?œá]ÛI?¸8ˆ¾sü?ïõÕÅÖ?¸8ˆ¾sü?"ñVÃ%ò?ìó;³?ïg u€à?ìó;³?aK"aÔ(ß?I`Ùì)Ö¤?ïî´liñÇ?I`Ùì)Ö¤?/Db¦ì	°?'Xã
|´?ïþ¹û•?'Xã
|´?…[˜o1—ü?¥	'ÀT?晴žþP?¥	'ÀT?…h˜
á½?†IëeÒm?ïª]Ÿÿu}?†IëeÒm?,Üeð?…¶? ®mœm$Z?ïþ29Ûec? ®mœm$ZPSR3FGL J2030.2-0622@CUv?ø="À8Û[¿CwNÀ9C†åaïÀ;[?ep!?ÈýWlÈÎ@'5·œäÓ@ 6à'Т¿èOÂ)I"7¿éPH÷Y'¿âj˜2CýŽ¿äòŒ~ËY}AGNfsrq@"¼ýŠÚ¹õPowerLawTXS 2027-065?ïÿÔ´Ö>™>óî	µ[<>õ¥•	)·6>óî	µ[<?ï¥Qøè?š°_ªk–?†«Âp$?š°_ªk–?ïÕ…ÅŸ?}ž%BxVC?u}õJ+´š?}ž%BxVC?ïþ|¾}ºÒ?¨mnûfâ?(4%Ç$ð?¨mnûfâ?ïÿØ{yb>õÒrF†+>óþ7/rÐ5>õÒrF†+?î,2n…«?»2>|Θæ?­<ßÉóŒQ?»2>|Θæ?ï¶ØJ²?¸.Õâgl?'z	ùÙk[?¸.Õâgl?ïúŸ…Ðä?;wT|¦?Eêù¾wÚ?;wT|¦AGN3FGL J2030.8+4416@T–Z?çvœ@ößoçšÀ7«ö©?)À:|^ʐ²j@©'¿šÃ@ã$ð_?ûé/Ï%—"¿Ôd=eÕ፿â
ñ!bGÀ¿èa9çéo¿ï·},¦|+PSRPSR@˜ö쿱[WPLExpCutoffLAT PSR J2030+4415?7)"ñ궓?3¶\p2àÚ?ïýͶ¬¥?3¶\p2àÚ? •–¢Èæ?¹²haW"?îö¦ì˜"?¹²haW"?"Û¤RôÖ?'-™i"°?ïY"ß0°*?'-™i"°?j×ë!–9¨?Ra
Au*û?ïå(éh†?Ra
Au*û?=ç;‹zÍ?4n±ñ¬ke?ïüCŠOO?4n±ñ¬ke?"àE&ZÂ?¥çNŽp€"?ï¬~ëÒé?¥çNŽp€"?v)ø,½q?sŸ"Ce#?ïÓ¬›‡
?sŸ"Ce#?4ô0#îL?%֙GÙ?ïý¡d­î?%֙GÙPSR3FGL J2031.0+1937@O( 2:À'`ÿX±À9¯˜JAÀ;o7…¨K?僧GŠ·@ÇJ	
šÈ?ý5ëˆ"¿ÛãÅñ«_¿©;!ØܔZ¿Øð8^¡`¿Ú·Ñ‰[D0AGNbcu@­½$%®æ2PowerLawRX J2030.8+1935?ïßa
B4i?ª(Áå€?pOzÆ(›?ª(Áå€?ïn»Ô¤Sÿ?£$øÀ˜!z?'(…m-N?£$øÀ˜!z?ïÊXäG½¯?zÿdÍ}­p?zӍéߘ‡?zÿdÍ}­p?ŠnÀ?hïɤ•ËU?‹Õ]›Ø?hïɤ•ËU?ïÒlå—R?w²$ÿ`—H?vÉòsg%?w²$ÿ`—H?ëöî/·Âh?Ä`lŒK±?À$GA ö_?Ä`lŒK±?ïRc§;»?Ü>X ­?•³‹©f9?Ü>X ­?íÚ¸h'T?—dsè?±*?‹Ÿ_?—dsèAGN3FGL J2031.8+1223@LÈ bÀ/mÇÀ'áÀ9Kƒg(-FÀ;4ÎAAð?Ô¥}}a@§ÃþÇò@yF÷¶¿ãQßy¹Õ¿åŧ(Zà¿é\1'&ç(¿ÝôÌõUpåAGNbll@'ŠâëC-PowerLawPKS 2029+121?ïüæ¨k¨?@R ã¦ÇÖ?8'¨?@R ã¦ÇÖ?ïjOw•"?§š!#Ù¡?'¶5å‡?§š!#Ù¡?ïÑQz൧?rºWÉÒ[×?wWB"¦l¸?rºWÉÒ[×?ïç˜û?Q*ÊêV™?hg­w°?Q*ÊêV™?ïñwg¦¾?f÷³xƒ-?]1(µŒ"?f÷³xƒ-?í<œâ_—P?¼ÎõºO?¶î»z?¼ÎõºO?îõ™ƒ¸öp?—˜Ã¾'Èw? ¦gÄp™?—˜Ã¾'Èw?ïzàà™Í?½…€3ÌH?ð£à}*d?½…€3ÌHAGN3FGL J2032.2+4126@T
ýòÿf?ðMô·ÍÀ6'•¿†À:ª¡(Ú@ðzú;J@
*÷%æÄp?ü†!'Kòr¿¿KŸ:ÃJm¿Ù¢#ÏN¿âmA'3ÿê¿ìY!d(ÉxPSRPSR@˜`éᰊPLExpCutoffLAT PSR J2032+4127?"£ïßz'+?&_ê$'?ïþÕÀç;c?&_ê$'?¤E¢Ý¡B?À,=W›¿±?¥Ò%ì?À,=W›¿±?Šå¨òÅ2?­ø;7?ï—üi%;,?­ø;7?R§+ª%Ô?@vœ˜&?ïö¬j_Lõ?@vœ˜&?60Š]r?.2â!)€#?ïý.Yã(â?.2â!)€#?‰']o"¸°?©Á1½Pÿ?Šk(m?©Á1½Pÿ?w#>‹èiS?sÔójÐîA?ïѹ'åo}?sÔójÐîA?'Žî5e1?!¦«£­±–?ïþ‡øB>?!¦«£­±–PSR3FGL J2033.6+6309@XŠ?ÿÊP@*þJ`vb]À:k£¢1ÐÀ;Ä×09¿"Þ#õ‰¢@C@1"J?þRa~Ë-¿êÌÀl¹‰¿æ"Û|	ˆ6?–Š-júÓ¿ÖŸjO:aAGNbcu@µÛó÷ÎÙPowerLaw87GB 203249.5+625814?ïÿ^³U)?çE™ÞMâ?)Ÿ"Yl?çE™ÞMâ?ïÎ5`)Ù?ƒ;ÕÈå[?xå@]©ƒ?ƒ;ÕÈå[?ïçm'T«Ô?aÚ4$Y?h'mšÖ>?aÚ4$Y?ïø¸ñÏ¢?7;ù
§ Ô?Mœ"Ÿ>¿?7;ù
§ Ô?ïþ»a6óÿ?!¶S #i?$I둩×ý?!¶S #i?î£iÕ9`|?µ0—
jz1?¥Ébª²*;?µ0—
jz1?ïސƒ	N!?q†",y?p·¾oªCs?q†",y?ïØ0ŁÄ?l½žmÖ'®?sç𩝶?l½žmÖ'®AGN3FGL J2034.3+1155@L?› 'À0|rŸYÌûÀ9±vfŽªRÀ;wœÏÛ?åŽJݍ©@ÅÆ"8@̵ `]8¿åq¸ÆýÍB¿èÍò¢Ûré¿æ÷£"Šú¿å†>•^mìAGNfsrq@—Ÿ8 -àPowerLawTXS 2032+117?ïû¤0vjk?\Ž©P›ÎÓ?Ao> bè?\Ž©P›ÎÓ?ïH
éUL@?¥AÑ$®?–þBÑæÛú?¥AÑ$®?ï–Êá~úK?ˆ€ì9#¸?ŠMG AmL?ˆ€ì9#¸?ï´2^nl½?d"'b(—5?'óhj"Ô?d"'b(—5?ïéa™ou?‡þH}™Ê?fïž5+ ?‡þH}™Ê?ì$a1¯`¼?À>4,ò?¾Üör"ú?À>4,ò?í"DÓøÝ?¦s2˜&Ԋ?³]Ù^?¦s2˜&Ԋ?î®oÙE›?›°Dù%¾?¯õk¦R?›°Dù%¾AGN3FGL J2035.3+1055@K°‹ßœ³*À1;`c'À8ihÎör¹À;'ÃbÀ¿x?óÉ®	h4@¼0V½@¾4à1ƒ†¿á'Zr^¹–¿æ†?"ë_	¿æ´KÀÈ¿êAë1^>FAGNfsrq@ˆÚâe,PowerLawPKS 2032+107?ïú"Ÿùsä?D>¼Ž¬'?E­€÷0ê
?D>¼Ž¬'?ïLÀþZ9?¯Ú¥òþß?–gýäTë?¯Ú¥òþß?ïlò%ïT?‰	þ4Á?'a»>¬yu?‰	þ4Á?ïÆ«ŽATg?[³þJjH?|ª8õSLƒ?[³þJjH?ïó[Ëòv?T§¬A?YHg¤á?°?T§¬A?쇢V#‰?Ã3-BÈ?»Âï5Nãµ?Ã3-BÈ?îèb¨Òؼ?—ÿ&ªþ_±?¡yÕp>¿I?—ÿ&ªþ_±?ïR@x&h†?"L?)Ó¼j?•·ðù{!L?"L?)Ó¼jAGN3FGL J2036.4+6551@Y(¯ ê[S@-ÒA³ÿÀ9¶ñµºaÀ;¦‡dã¯?âG»){_@¯^ìI"É@€-?¿áDˆ¢V=¿à¢8±ø50¿Ó¦ã¬ë¹€¿å‰_ț|AGNbll@¦ŒÒ:)ÇzPowerLaw87GB 203539.4+654245?ïþeŠ&?+6$©ù z?)§S[Ëø?+6$©ù z?ï»[­¸³?…^
zÂ?)Çu?…^
zÂ?ïë8ÄRæé?V¸Zêÿ2;?dÇ;­?V¸Zêÿ2;?ï|z(Sõå?m´µˆ8Ÿ?pºõCY?m´µˆ8Ÿ?ïðÀœ_> ?bÕ.z!¾F?^~ÇTÁ?bÕ.z!¾F?î‰bPx?²›h?0Kà?¯‡iܶ¦z?²›h?0Kà?ïµ+»š U?†üìþ…&|?'µ'nPº?†üìþ…&|?í*ËÛ»8?¡» H˜Ö?¶©¡'?>?¡» H˜ÖAGN3FGL J2036.6-3325@#X+€~
ÀA½â:¸cÀ:žƒujæ(À;£Ýs
=Ö?æז(î-<@
–B	òa?ôàÓËr/?íš|˜ì¿ïïrȖÕ?ï¸t´™
?×K;IÕAGNbcu@ÓÝp£×
PowerLaw1RXS J203650.9-332817?ïøþÁõr?U%è×£J1?LìÍÕn?U%è×£J1?ï»ggËÉË?šò[âë˜?&&ÞAC?šò[âë˜?î4‰åF–<?¢lJTW³*?¬·a¯84?¢lJTW³*?ïýJÂW93?7¼·Ý_OV?5©ìÈÞAÚ?7¼·Ý_OV?ï÷~Ü÷4?`+Þn¢'q?Qù¼¡9)?`+Þn¢'q?îÝ¥ux…«?±ÁÂv•Z?¢%¨¥	O?±ÁÂv•Z?îÐçêñŒ0?™Ë™'-Ó^?¢ñQÃ#þ?™Ë™'-Ó^?ïþH}©Ï?2Ts‡¹:?+v&ŋÚ?2Ts‡¹:AGN3FGL J2036.8-2830@/Êœ£9ÀA2¶­À9·'%VўÀ;ªÀ:ñiš`>F@í-–¼¡@ž˜›ü ¿â´låö-]¿å¥F‰Yä¿çÞùÎ@G÷¿çe±jFAGNfsrq@'³ˆ˒:PowerLawPMN J2036-2830?ïþôf¼?×4€èǒ? ¹"í]T?×4€èǒ?ïÍ\«ÁS6?'Šù‰<€ï?yQª8"ø?'Šù‰<€ï?ïÎY†ÑbU?uh\)ÿ?xÓ<‡€¡€?uh\)ÿ?ïÿyez5Ú?O	FsZÌ?ÓMz	´`?O	FsZÌ?ïþ)ÖNg?1ñ±MŸV?/}^n_âÑ?1ñ±MŸV?ïÒÊÆ?ó?­ýI~=?žå¦¬_kŒ?­ýI~=?ï{W[¨ê'?‰˜Ùiäb?•Šâ­Æ?‰˜Ùiäb?ï÷â¾aá-?IÑéåN?P:ƒ
'öÈ?IÑéåNAGN3FGL J2038.8+5113@V/×,uª@Ò½ßôò±À8˜ÈQ=	vÀ:¯ÚM¾Ð¿ü"ƒèØF@ŠÆóïÑ_@!ÙŒÂÇ¿è~3•6f!¿êö°Šï);¿èó"ëxš­¿ç·Õˆ¡éAGNfsrq@v yÛ"ÐåPowerLaw3C 418?ïÿi¬Ž`M?qN ™@?Êhú¢m?qN ™@?ïÌj	"?ƒÃ9,%?yõÊú'G?ƒÃ9,%?ïI¤ÂJE|?"o	ޝ|?–Ëg´ÿ'€?"o	ޝ|?ïÿù³ÆҞ>ÂÐß¹Ün>É0QðØ6>ÂÐß¹Ün?ïüg"_6­?C\B'zÓå?<Æëº="ß?C\B'zÓå?îΡÒ^mZ?¶[&s0?£âÛÐø`?¶[&s0?îCB{`ڜ?¡26­íâ½?«ËØJÎ=7?¡26­íâ½?ïÿ(òèj?m±ÃÕ?µ¹o"?m±ÃÕAGN3FGL J2039.0-1047@A£Rÿ" À<½ÜŸ¨§TÀ8¼äÏøÑ8À;8E­‰:§?÷8(Øîn@£$¨«Û;?ù§´³Pz?§†õŸv¿à:3Ïݛ¿â}zvÒ¿â7è6;6AGNbll@Û«¹Œ~(LogParabolaTXS 2036-109?ïýNZ‰–ö?2·qoj?5-	;
O?2·qoj?îàR%Ü?­»5ŠKT?¡÷êÛ÷$I?­»5ŠKT?îi–ÕwžÑ?žèInÍ­?©f'¥vû?žèInÍ­?î3{^w…?‰…[%ÿ¤?¬ÈJ!°U¨?‰…[%ÿ¤?ï÷­?=Ø?Zf!ƒ›ž?QÂ¥!O?Š?Zf!ƒ›ž?ë$h^Ûz?Ãðk3:ü?Ãn^"'ç?Ãðk3:ü?ííð)%ò?¦$ˆrK`?°— ~¶Ðr?¦$ˆrK`?êIÃb7O?­ÖóÎ5°ü?ÆØòw"Ü?­ÖóÎ5°üAGN3FGL J2039.5+5217@VkΠ£¢@
æO†%À:'r—ÍÀ;_®FÏÈ*À7Õñ
ÉÂ@
Z×h\4ß?þGàðñ?ÜMâ'QåŒ?ëHo«¿âP¸S¿Õ¦Ð†73•AGNbll@¿M¡aä÷fPowerLaw1ES 2037+521?ïúߺeA"?oʥ騷"?DŒTǸ?oʥ騷"?ïԃŽP¡i?'0
µiǂ?u¾8·b÷?'0
µiǂ?ïÆøÞYu?w_és›^
?|ƒ'¿Ás?w_és›^
?ïÿÿžÓŒ§>"Þ¯m8a<>ˆZ>É2>"Þ¯m8a<?ïúéL¬£Y?EmÉí?DZÌW´ó²?EmÉí?îüée'^š?±9"x';? 1i¤Fa\?±9"x';?ïêņ:?ˆž,ßŲ?‹ÅNÈáN?ˆž,ßŲ?ïÿò­ËÄ~>çED¹Î=M>Ú¤EÕB)N>çED¹Î=MAGN3FGL J2040.0-5734@u:jŸ{ZêÀB‡ŽèӔÀ:O»¢çÀ;¹Åԋ0¿þî5'³÷>@
ú…\ '@'Ñ`w‰?휃OÄþ¿éó£ËC,G¿Ö[âé2¢Ù¿ìK%99KjAGNbcu@™=p£×
PowerLawPKS 2036-577?ï̞ÒúŸ?ŒRM•ùÁ?y°–Œÿc?ŒRM•ùÁ?ïÍlô\?rû—8â?yI…ù2j8?rû—8â?í`L'æ‹?¢bºžó?´ý›ðJ¦#?¢bºžó?ïÿæàÒÆ¿>çˆï)Þy>éÕ»>çˆï)Þy?ïì" f…y?k‰žk¼ÄÈ?ckß]v?k‰žk¼ÄÈ?ï "ސ?³Cs^鼿?žëÿ¬_÷?³Cs^鼿?î9b|?¢lo~Û"?®ìr)t5?¢lo~Û"?ïþš6w
?&s¯jÆîÞ?&\žrkg?&s¯jÆîÞAGN3FGL J2040.2-7115@t2gŸì™òÀAá`xÀ9§™hò1áÀ;†‰1l‰–¿×ñÆ<Ÿ@
Õc¥ì¹&?üÃöM½ù¿æÔcGß"÷¿ÕŸ–äL_¿Ö˜÷f7±¿ÑèP©ï/×AGNbcu@¯–ç-PowerLawPKS 2035-714?ïüAE´Xü?6ì4 Ñΰ?=õÒÂ_Ϭ?6ì4 Ñΰ?ïͽ.†^?‡rÄ{l?y!hí>±:?‡rÄ{l?ïÕcøß
£?t¼?$ÇÏQ?uN|Œò…?t¼?$ÇÏQ?ïü°?)á?'–<VêV?:ÝpáÇ?'–<VêV?ïúgғû?Ar!œ&?Fc©;GJ!?Ar!œ&?ï-–·ÎB?¬Ò‹F¨WŽ?šM)<7Ç?¬Ò‹F¨WŽ?ïÂÒG,†¾?BÚÆ	º?~–ÜbÝhþ?BÚÆ	º?ïÞÃø4Q?eŒ?agj?pòb·S?eŒ?agjAGN3FGL J2041.7-3732@gE_ۇÑÀBš$€	À:w$ú‹LÀ;—œ`ô6ž¿æ«ªùÆÞ@
¹« éð?ü™Þ¸Ý'?ãà¶cÁ¿â·£??¿ä\ÓÚL¿ªwYƒAGNbll@¶¥
=p£×PowerLawNVSS J204150-373341?ïþM˜}ÿ?/~ êuÈ?.{"åTÚ2?/~ êuÈ?ïÃ&Á½¥?™9Ø´y©@?~lô"‰ ?™9Ø´y©@?ï…0	C[Ü?Š‹©â #?Ž³ý¯)	?Š‹©â #?ïÿ'ê&-?ݲ¡w?›Éס¹?ݲ¡w?ïüÞÜU;?>‰qÞ°¡?9	0@hg?>‰qÞ°¡?ï@z6°sÙ?¦¢jKñ÷?—ð¹(9¶Ù?¦¢jKñ÷?ïP%@|ó?'Œ˜Y?•ûP)±?'Œ˜Y?ïú]Vt?J+AUïx"?F‹²Új¯?J+AUïx"AGN3FGL J2041.9-7318@t
ÀÓgÀ@Ýn˜K¼À:¬(©lÀ;ɨÛUüŒ?óVµ"ö@Ë$Np@­œ€~Àz¿é«-ˆ×Þ¿ëM‡sb‰s?»fpѓð¿âw ‰s—ãAGNbcu@žU¿—$tTPowerLawSUMSS J204201-731911?ïðõ›£	/?c'ó¾ìÍé?^ÈöfÁ±?c'ó¾ìÍé?ïÕ}±—Î?¦Ó
+'D>?ŸEPF]j;?¦Ó
+'D>?ï-‰')Q¢?'ɉ)¤Ì?šN͹ýÉ?'ɉ)¤Ì?îš|Y( —?'­ò?¦X:p풐?'­ò?ïöÑbU,$?f­ù¼ÒÏ?R];4«xª?f­ù¼ÒÏ?çÊ3|¦'?ÐF¹¢Îw?Ðk™²ÝÊ?ÐF¹¢Îw?î""ÓÙJM?ž€·`Ùþq?¦ÍÒÅÚ÷$?ž€·`Ùþq?ìDZ1;?´—ǝ¾
u?¼Ç*vv)?´—ǝ¾
uAGN3FGL J2042.1+2428@PòaßîèÀ%–Ä!, rÀ9ÓpàÓÀ;†3çÀ½¡7Ì¿@Šþ@8ã?ýß#ÿŽ–¿ëi*Ý4Š2¿Í'«é[Š¿Ôjë%¨[(¿Øb' 4AGNbll@°P2£S&PowerLawMG2 J204208+2426?ïþª,¹Ça? {ˆÀ½›?%]4¿åÎ? {ˆÀ½›?ïÀ@%EE?Šl¶Šá²ò?ßío;m†?Šl¶Šá²ò?ïèddGl?TàZßÑ·š?g››ó­3š?TàZßÑ·š?ïÿÿÑJÏ¡>'²€me¤>wR3—}9>'²€me¤?ïûë.Þ^?:TÿúUÒ?@SD²«¥ö?:TÿúUÒ?îÁ€Ù.Z?²†Hª6÷m?£çòhÎÜ®?²†Hª6÷m?ï×;|?u¤:"ê?tb´]­ï?u¤:"ê?ïÿûï‹Nä>É×">ÀA'Å.}¿>É×"AGN3FGL J2042.1+0247@H?÷fÔÀ6ÿ n4'À:Y)ªIëÀ<:&1Âð«?ù)Õq6#(@
É, ð:?áçy©í­¿ËZfØ1¿Õ!÷'"b·¿îOÙGÀš ¿ßk;Õ:¦çPSRPSR@'b¼ÚQLogParabolaPSR J2042+0246?ÕÔü½?Ò^iIg•?åtý~¡?Ò^iIg•?ÐfIQþF?ѐf)ªžO?çÌÛWv€Ý?ѐf)ªžO?â"/Y?¶µu6E³Õ?ÚÙýàåO?¶µu6E³Õ?Ôå!‹ôs?ºàygu9?åpo:Æ?ºàygu9?Ýœ0!ÛÈ?ÓÏd¢þ‹?áy±çï?ÓÏd¢þ‹?–ÀîˎÚ?ª*ÿ$?ïIø‰¿?ª*ÿ$?ä]ý_s¢?¸á.DD?×DAͼ?¸á.DD?›"/,Ææ?¦ñw—ŠL?ï#ކހÿ?¦ñw—ŠLMIXED3FGL J2043.2+1711@NóK 'ßÀ.šDÀú0³À88í¥,uÀ;I»	Uê@¦óp.@Q	@¢C@Èx»¨'¿×܀"'(}¿Ýk'oŸcø¿à«ƒ½u}¿ì«Àã†PSRPSR@Žˆ1&éyPLExpCutoffPSR J2043+1711?`9֊@®B?gT¶®g?ïïÆ)£)?gT¶®g?¥¯³Y?½¸Õq¿"?î¥"Šò@?½¸Õq¿"?º´¯Ü?§¨àä?ì©J}`?§¨àä?ª
Q™?_ú=R®¿?î_6/M0Ç?_ú=R®¿?b‹0c_ÌÊ?\ ô}ÔÜ?ïítÏ­S?\ ô}ÔÜ?"0=Ê
ܚ?°äDìŽÌ?ï^~Ë%û?°äDìŽÌ?›&»šd3 ?'°"ßÑ í?ï&Ê#q–"?'°"ßÑ í?…mÑèá—?y"€žÑù?ïªH¸wø?y"€žÑùPSR3FGL J2043.8+2741@Q¨¸!ïÀ"NîÀ¨tÀ9*AÖd%DÀ;ré?û1Œ$;¸@dóiï‡ã@4J´RE¿Ö…<6ß\"¿àú¼Ê J¿êia@óÌQ¿îÚâvy¦WPSRPSR@…×0¾
íPLExpCutoffPSR J2043+2740?©Q¶?«þC±=vÄ?îoªïú›´?«þC±=vÄ?°Ú¶ž¦ãs?ÁÅ2ñç0?íä©,+#'?ÁÅ2ñç0?ÔD$"NA?¶ç£ÞY ´?åÝíµ¿Xà?¶ç£ÞY ´?Ãzx ™?›ñ0%?ë!aþ¼wÚ?›ñ0%?`"I†.&?c·¸Àˆ?ïï{¶¸A?c·¸Àˆ?Ëú³È–s?¥˖	úÒ?ïy *Šöœ?¥˖	úÒ?¡m"}Ú?›—#\Kfx?îé&¸Y*ò?›—#\Kfx?†¿‰Äð?t^L»ÁH÷?ï{ςpH?t^L»ÁH÷PSR3FGL J2045.2+5026e@V06â—@®k³¤ˆÀ7"S‹˜OÀ:C/(·Ä@¢ó_2•@G™E`Ý;?ýÆøÒ¿Ï©0&Ž¿äùÄ÷k¿èƱ?R¦@¿ìÃ"Ê/c›OTHERSNR@'¶m'hr°LogParabolaHB21?eˆ[$/1‹?llÞ Â×M?ïêw¤ôþ?llÞ Â×M?¤;ì¨$ñ?¾†ï2}?î¾üAPú'?¾†ï2}?ª5RÚ-ã‡?¡ÿÈa?î\ªÒjà7?¡ÿÈa?‰ùKZ×`?qk²ºTµœ?ï˜ÓëÏò?qk²ºTµœ?\ÇÑfÇA?]íK‹,c?ïñœ"[u?]íK‹,c?N=¨!à?©Í£Ûh¦E?ïŠÇªà$)?©Í£Ûh¦E?—!Clr?—-ýÌñv*?ïGGGa|?—-ýÌñv*?]%Ìê23?P+ïá?ïñm*o?P+ïáPSR3FGL J2046.7-1011@Bl@%NÀ>2w"^À:jSâÖ#ŽÀ;"bۗjë?À'@"ɝ@ŒV¹ E?ù¿WAï9?ïðª(¡Î‹¿¾½mÍx¿×."Â3/œ¿Ï$ô'IÕAGNbcu@½8|~($PowerLawPMN J2046-1010?ïþ;»~,?'U·9ÿwØ?,DL:"ö?'U·9ÿwØ?°åKÛ?£Ÿ;Š"Ã÷?ŒV"Ôky6?£Ÿ;Š"Ã÷?ï´ùÿô†?ûÞÔ}n?'Á˜qìx"?ûÞÔ}n?ïó8{À–?C˜ Ìóöù?YŽü¥Š&?C˜ Ìóöù?ïû(#ypž?Bûw¼Æ`Ÿ?C_q÷T·?Bûw¼Æ`Ÿ?îK8êº?·eH=¸E¢?«L~"âd?·eH=¸E¢?ï{§Af°?‰©Ò¹Û4m?‹ÛBÅó?‰©Ò¹Û4m?チœ'Šp?t±±›G‰v?€_˜ääUà?t±±›G‰vAGN3FGL J2047.1+1054@Lˆ)³únÀ3¦Ÿä6vÀ:\l6‰ÿÉÀ<,)ñk?øyȈÅ`ó@-zØcXë?æʒéYÔ?îËa¦Üi?ÄOð Âv¿à"¥…¾¤¿í¶™£ÄY¥PSRPSR@¤•Á½¥PLExpCutoffPSR J2047+1053?›æV§&#?³JVª†?ï ÍO©‹?³JVª†?ÙáÐ
€×?пõÁc?ãú¿ñ"?пõÁc?Ö	2Ú®óÚ?¸ýî"2	?äûf'¨†?¸ýî"2	?á³çc&?´(­›"?ܘ19³ÕÛ?´(­›"?"ú&ªÂ>‡?¯õO0–€?ï`.Ê©î?¯õO0–€?ÊV­–{¬õ?ÍlùÙÜf?éjTšaÃ?ÍlùÙÜf?Áólº¤'W?ºA¦F-êR?ëƒ$ÑVÛj?ºA¦F-êR?Ëx¿"€¼?³/Zø;hö?é!Ð<÷_Ñ?³/Zø;höMIXED3FGL J2049.0-6801@tj‹@p2˜ÀAò¨`úÀ:%êIµU¸À;Ä)Ĩb?åæ)Aí¶&@!Úi˜u@xÓ@Yap¿íƒ˜í»ô|?ÐìMë	<®¿â§ým‡¢¿åGqaIÐAGNbcu@¤Åú^5?}PowerLawPKS 2043-682?ïþÿ?*§°1öµ?/À^³¸?*§°1öµ?ï¤vŸ×Ä?'30¤LK?†â{åÈ?'30¤LK?ïÔX&µ?u(‹Kb}ó?uÓü?ûÉ]?u(‹Kb}ó?îƕË%O<?'ò%«Œ?£–£Q¨7?'ò%«Œ?ïú˜Ø( ˆ?DÈ
ȏ	?Eœ uûO?DÈ
ȏ	?ëÐTßÕ?Â}½M±lR?À¾®¼€­?Â}½M±lR?ï‰lü5MÈ?ŠÏ®Ÿ'\—?¤ÁjýÞ?ŠÏ®Ÿ'\—?çÄV¶1!?¯÷ª*'N?ÐwSʓ½?¯÷ª*'NAGN3FGL J2049.7+1002@LWú€d>nÀ4­€'ÍÀ9=A&QÀ;|v,­5?ÔSÑA@j•pj @9Ûm¿å\'"Á¿æÑX«Eq¿åÇiX¿ç‡ëÕ·¾.AGNbcu@Š²€hۋ¬PowerLawPKS 2047+098?ïþbDŒ?7ˆãçV?)ßÂ\êÎé?7ˆãçV?ïz½¬sf? nF&Òh?½HEJ)G? nF&Òh?ïÖa=)"°?rÓq¸~?tÏaTÁ;â?rÓq¸~?ïÕ«"ƒº?XÞ\çý?u*nÕ'º?XÞ\çý?ïõt¦…e?a뤡.?UÔ¢wc?a뤡.?íóÛœB?½îfᜣË?·ha'ãò?½îfᜣË?ïP`bÜÕ?"ž÷Ÿ?•óóºôÉp?"ž÷Ÿ?îªIþYj]?¢!5þ?¥[`Øö)?¢!5þAGN3FGL J2050.2+0409@I·PÿÌÔZÀ8t-݉À9Ø
¨_/À;"8PÍx?ã<ð×v§…@
$*ÌÝ=Þ@‰¨f翕ЉÍô•¿à4Õóo¬i¿ÝmyzÀ:˜¿æÈŒ·€WAGNbll@ž#­BÃÉïPowerLawPKS 2047+039?ïõG/>†ù?d¡A6v÷?Uq¡aõÍ|?d¡A6v÷?îõ;Ó·^?¡3¹TšÃ? ¬BÏĊ?¡3¹TšÃ?ï·£'Á¹?yª»¿…â?'\HF"?yª»¿…â?îOÑ(üùe?…û\«rL2?«íqè7¨?…û\«rL2?ïo™¿?±?–ˆ3\ýÃ?'ÈeÐ?–ˆ3\ýÃ?çÜÙMfÒ?É>¢¬V¤k?ÐFMeÓ2[?É>¢¬V¤k?ît_SÞµ"?¢4ÊRç_?¨º
ńBÀ?¢4ÊRç_?梥¢Í†?°²ôºu³ì?Òº´ºdóÓ?°²ôºu³ìAGN3FGL J2051.0+3040e@R¿íÁ9À! ÀŠÀ78IqcÀ:ŠÂp@°1a÷ÁÃ@òäñܦµ?ýÜSûª°Ã¿Ðþ¯¾3G¿ãlˆÌ¼¿åSºÇ犾¿ëÈeÊ_4COTHERSNR@å!WhLogParabolaCygnus Loop?tMʯ(\?wõHÀÞ?ï×e蚼7?wõHÀÞ?¥º¦,ð'?¿¢äW><?î¤Uz?¿¢äW><?µoæ"é:?¦o[…d3?í^ò=!I?¦o[…d3?—ì£È?Ëý?~­«oêÿ?ï@šá‡à?~­«oêÿ?YRõlêi4?UôŽŽIî"?ïóV….
ì?UôŽŽIî"?‹oäêOêy?¨UOI‰?ï'@lVÀV?¨UOI‰?šP´G?—^{
L¯?ï+Ä~?—^{
L¯?kPP(ýZ?^¡Ž^Ò?ï䯯°‡G?^¡Ž^ÒPSR3FGL J2051.3-0828@C™* dúVÀ>v |wJÀ:yö£•œÀ<FÁƒÃn?ú7¸ék@Ë»O†¦?æ¨Ì]Ÿ÷?ïÿœ)''?ÅýíÍž¿ã4Ìå^¿ïÿMfÿØ,PSRPSR@¢ÅCþ\'ÑPLExpCutoffPSR J2051-0827?£ÀMÈÁ†?²ß@¢¾y?îÃû#f%h?²ß@¢¾y?Ì#üë?Ͷkr¥ö?è÷8{ûÅ?Ͷkr¥ö?Ï^/ž†Æâ?·&­kÛÐ?è(t^NH?·&­kÛÐ?Õ-"Ãä[?³?áxr±?åi6
öÒ?³?áxr±?¨W'""¢i?³]¦3*Ü?îz‡Ý¦Ü?³]¦3*Ü?ÀGÖI^~ø?ÇMӝvrù?ëî
m¨`B?ÇMӝvrù?ōs)(©?¸ú"þõ?ꜘ£5µÖ?¸ú"þõ?´ŸÿF>B?¢—Rï'n?íl8<?¢—Rï'nPSR3FGL J2051.8-5535@u]Ø`fÀCx) zbÀ9ÔûÔ!TäÀ;¥°a\;j?ÇÞ¼Eb'#@ã'ÎQ@ž^ qº'¿ë ™¸Md¿çúË¥ÕE¿ÜqtAEo¡¿àGŒ5zW¬AGNbcu@‡
¹=ÙcPowerLawPMN J2052-5533?ïÿèÀÉ3e>å0…F¨UÄ>ç?+©§š>å0…F¨UÄ?ïÑå66Y?''PGƒ0Ó?w
dóñ¾?''PGƒ0Ó?ïç&A:æ?gn(|øÛh?hðقKùð?gn(|øÛh?ïû~ÞØ=?&Åks%'µ?B"ÚøO?&Åks%'µ?ïÿë{Ê·Û>á´ÆÃœË>ä"i4rð>á´ÆÃœË?îúü/»Úa?µNëHÙzÀ? P=®¤ð?µNëHÙzÀ?ïË´"JÇh?~¾@¢ôj'?z%îíÚ¾?~¾@¢ôj'?ïè«ö–[?Vœ3"?gT
/b%?Vœ3"AGN3FGL J2052.7+1217@MŽnß±«ßÀ4ù@ÉìÀ9Á+KÞ$äÀ;˜†1		?Þ"ɘ\O@
TŸãŠ©@¿ÑÔ¿àÍNnðE¿ãQ'KŸ:ÿå4'౟ä¿äùÿäþ›PSRpsr@"ÖMjOPowerLawPSR J2052+12?ïýš"/;F?6ÏÆÁóU?3+] Ç?6ÏÆÁóU?ïxç6ÒÇZ?¡Fs%í?ã'^â»?¡Fs%í?ïȗyask?xq‹|Û%á?{´Ccãò\?xq‹|Û%á?ï=µ?~Œ£Jsì?žø]D4Õx?~Œ£Jsì?ïòn
à?`@£8¶5?[#æ P³?`@£8¶5?ì#ÎjÔ?Â=* « ?¾çQŒ©_ú?Â=* « ?ïK¯Ä†à¸?'ç'ûä %?–Šr""ý?'ç'ûä %?çÊF"bH?²×HîÉÑ?ÐkÓrÙ;p?²×HîÉÑAGN3FGL J2055.0+0016@H9Ÿ C×ÆÀ;
v_Ø­¬À:xÊ J"cÀ;ž‰.‹C?)ÃZ<¤c@úׯ~Þ,?ûºb&%Ú?ïô>!gž¿èþúÔÇíë¿Ú°à¤a
¿›K§7µ"AGNbll@³Ò4`ªdÃPowerLawRGB J2054+002?ïÿ%ihpÏ?·´ÞêNT?RØ&É
?·´ÞêNT?ï¤S_+<L?"Èû'þß?†ë(.Q´ï?"Èû'þß?ïÏ®…}Ǜ?o¡ƒø‰â?x(½;œÒ¡?o¡ƒø‰â?ïýø"hí?'ëЪ·›s?70;[sø?'ëЪ·›s?ïþ,Ëåò
?2v.m¥?-3EËeíc?2v.m¥?î#Ꮆù?½#ÜWsH?­Îaë`o?½#ÜWsH?ïŠH‰9WÃ?‡4Ë Ç˜?mݧ[;J?‡4Ë Ç˜?ïíXëÔyê?^üè''	4?b§è-¾?^üè''	4AGN3FGL J2055.2-0019@Gó¢`¸À;hT`ªdÃÀ9ïtŠ˜À;cÌütð?Ü —8°•@hcJ?ùÿ!@AŽ–?o=òÌ¿¸íý^C¿Ì®ÅG>пÓm•¿ÅRZAGNbll@º5ÔzáG®PowerLaw1RXS J205528.2-002123?ïýä²Ð*?,«ÛÃ?0Új6NA·?,«ÛÃ?NkÑh?:`Þn<?ŒÞlv9±ì?:`Þn<?ïΑ?%?sôèÎÄ?xž·‰nQ5?sôèÎÄ?ïæ$¶Sö?P7"Ž'W?iëÛWjz;?P7"Ž'W?ï÷äÙf–À?O‡BiW?P6L¿¥þ?O‡BiW?î2 Þ~ÈT?¹Ÿá?¬Õòïa¹?¹Ÿá?ïŽ7™Qþ®?ˆ«0J­.?Œr¨¸‡?ˆ«0J­.?ï³åÂö?rÈv‡å ?ƒŠýŠ?rÈv‡å AGN3FGL J2055.8+2539@Q¬iöZeÀ)
¼ßÿ«À7 Ž]%uÀ;=¸·a+@~ÃS&m¨@JԏŽÔ?ûÄwÌk¿¶ÖĪ5ël¿ßc–éÍè¿éñ8‡¹zé¿ïÿÛrW
~PSRPSR@†p#̎PLExpCutoffLAT PSR J2055+2539?lÖå"/£?"	¬®ù˜?ïã)èÜ¢Ù?"	¬®ù˜?ŸªËX?·ì;~*Ü?ï©Þ5U?·ì;~*Ü?¡ÿ‡Ž
õ?—¿?¿ŠN`?îàôÝÁ?—¿?¿ŠN`?1üÂ`¯I? èHÔß-¶?ïýÝ4q? èHÔß-¶?qlû3›?ƒ"wuë/2?ïÝ&+ôâ?ƒ"wuë/2?Œ³¼(¼l?¨mÇpÑÖ?ï1†IŸ?¨mÇpÑÖ?Œúp°Š–?Š7¯ÂñnÒ?ïŒ?Ì7•?Š7¯ÂñnÒ>ýpÍõ»
§>ørP™œ?ïÿÅF€Ý>ørP™œPSR3FGL J2056.2-4714@v	k¿×ÀD0½ßÉÿ"À7HErÐ×ôÀ;|ê6j?ûü%íûE±@2ê
$@©³ûo¢z¿áO,²]r¿æ㺠^Ö¿çºg΁"û¿è;¤=XóYAGNfsrq@w×ûi˜JLogParabolaPKS 2052-47?ïü•­¯XÑ?@i"{‹v»?;R'z*W?@i"{‹v»?ïÂÂY<[?–+&¹J?~žÓ_¤'?–+&¹J?ï*µïYÇ?"€ËDöúÕ?š©BôÇ,?"€ËDöúÕ?ïõ¹NjÇ?DeÿqqR?Učpèá°?DeÿqqR?ïö.ùpLw?X©_wnRl?S¢
*'w?X©_wnRl?îžV:Qé	?»@d¾£?¦œWqÓm?»@d¾£?îç©uÀݑ?™×oÔSrÒ?¡…h¡^qì?™×oÔSrÒ?ïñ²œ—GQ?VëҋzŠ?\šÇh?VëҋzŠAGN3FGL J2056.7+4938@VSI`0Â@@ô´À;™ßÀ8ÖéÆ×qÀ:ågÉ<õT?é
"v"ÜÆ@[uLj'?üˆH€ø8¿×
Àي±†?ïýmaw¤¿×:CÀãϿݨSíN2ÏAGNbcu@¼&Ãn—PowerLawRGB J2056+496?ïðµ{2·t?WpXözŽ?^•	?Ûis?WpXözŽ?îŠój}?­R*ø~?§_@ÈÁ&0?­R*ø~?ï{'o†u¥?ˆBš%ÒïÉ?²XµJ?ˆBš%ÒïÉ?îg[aƒ0?"‹'c,Z?¯©ŠIçÌû?"‹'c,Z?ïŠVœ*(Ú?‹—⧂û?jXë&õ¥?‹—⧂û?é›Ð­ï‰?ʖêìâ/Ï?ɐ½K"AÛ?ʖêìâ/Ï?ï!²G:|(?•Yy0J?›É·‰?•Yy0J?èÝ¿I¨?¶¹Ùݯݤ?̋†Ù_?¶¹ÙݯݤAGN3FGL J2102.3+4547@UÀÇä¡Ö¿à	'€4\˜À9N‡"žyÀ;˜áãµG?ù°Ñì~@¡/Æl5ˆ?÷Kc-vÛª?´  S¿ã¯¥$W¿î£#á[¥¿é¼å~tz%OTHERNOV@QS&ÂLogParabolaV407 Cyg?ï"lK­¨o?¨z£'˜Ð?›²v'áø?¨z£'˜Ð?ïíÁ=?¢îGuÿCi?ZÀnY?¢îGuÿCi?勬€7Y?µÁüÊåm¸?ÔéЦÿ'N?µÁüÊåm¸?ï»± kQÕ?j̈eÂ?·Õ]VÖ?j̈eÂ?îMñÛ،?± ùÜ×/?«.0å²<?± ùÜ×/?í!™3Sz¸?ÃÛߺ:N?¶ó6ed*C?ÃÛߺ:N?æIãDC·÷?´Jt‹P?Ól9wx?´Jt‹P?ïkBG?"ím½Xø?œŽR¤Î½#?"ím½XøAGN3FGL J2103.9-6233@tË¡ ÏÀC{+ŸÀûÀ8è_⾦™À;em¼Øc?é90&³Û@Y–ù+O?ÿ›I?2É?¯Lùû%¿â¥—\[(M¿ÞLYy1Þä¿ãEÊ/ŽŽAGNbcu@™¨cŠ	PowerLawPMN J2103-6232?ïþo0±Æ?0ž`¥Y?m?)øèÄi«?0ž`¥Y?m?ï©Ï9íI?š	lõ¨Œ?…Œ1sŒáó?š	lõ¨Œ?ïËïË»ö?}y÷bV?z5uT®?}y÷bV?ïe®S¡#?p¶/Ó]"È?"J5'x?p¶/Ó]"È?ïý°ƒÚ¯R?3Îð£lՄ?2{à4;5?3Îð£lՄ?î+&¶fó™?·é'Š™'?­M"—Øøu?·é'Š™'?羽"1tä?‰#¾¹Ì`?…Ø^÷bÝ?‰#¾¹Ì`?í÷ˀ?šÝ_IÅ#"?·¿pEâ…?šÝ_IÅ#"AGN3FGL J2103.9-3546@aåéSÀD³, zûÀ9tÀ#i'À;§ò¼JžŠ¿Û÷øYÃjÎ@wçî@ç@GD¿ç	taÀ¿ä=t:ö‡¿ÛJÝQ‡å›¿ë²æë´×AGNbcu@ŠSß;dZPowerLawNVSS J210353-354620?ïøˆ23s?L:ºõ"]ú?MÝúxû	[?L:ºõ"]ú?ïÇ6Ù8ž‹?¡¨'$Ãq?|d"c°º¯?¡¨'$Ãq?ï8Æ&"=?f–j˜­¿?˜ç;,Ä
?f–j˜­¿?ïþìÜ%Ÿ?%èdÚû?!2<mÌ[?%èdÚû?ï÷	‰–—1?S7Ï´7œ{?Qììz۟?S7Ï´7œ{?ïh:~¬}?¡Ižƒ´'?'ø°%XFl?¡Ižƒ´'?îê™M2Q¦?—Ê¡!Ãâ'?¡Vk*G0©?—Ê¡!Ãâ'?ïúG"VMX?B
Æp§ÞÝ?Fá²Rx?B
Æp§ÞÝAGN3FGL J2104.2-0211@G°l_¤«FÀ>Hï 6kÍÀ:­ƒðºèŸÀ;²/ãšj?èÄàåç·@$+"Ãyg?øbIÿ''ì¿î86#	ð?ï²ؖO?ª¶Í±ú
£¿Ê]JÚùòAGNbcu@ÁAÐå`A‰PowerLawNVSS J210421-021239?ïü@c%÷?EbÖãP¢…?=ü觹¶?EbÖãP¢…?ï"	9([?— }Ôæ""?Žý±ÅU!T?— }Ôæ""?ï¢O#éû?‰ÍpÜm?‡l:}ä¹&?‰ÍpÜm?ï®ÿLÉ)?nþAý!?"yÀ0•GÈ?nþAý!?ï÷Ãy
?P"?ÇÔ?PyLõÄ?P"?ÇÔ?ìØ»¥T…5?Ã{×Y÷å?¹:"Õ[ÖY?Ã{×Y÷å?ïP×_'¤Ç?'ú!ø*ý?•å;?'ú!ø*ý?ïAÌõLÙß?Œ«KKA—±?—Æa[Œ.&?Œ«KKA—±AGN3FGL J2106.1+2505@QðMÿÒ³—À-\n>¡ü?À:íA·ZuÀ;âž43?ØR‹!J—B@žo}¼Ch@8©€—j¿Ú‰`&x:¿ë9¤@^p¿éV/3¿Õ€ùŸ¾¡¼AGNbcu@‡ î.±Ä3PowerLawMG3 J210642+2501?ïþÏ *œ%?&ý"óí¿‹?#ÿG8f?&ý"óí¿‹?ï£É»A×]?œâãX1m?‡
'6i`¦?œâãX1m?ï©phÁ?{f|ÎÂ!K?…£û˜_æ?{f|ÎÂ!K?ïç–wPC?SQõъð?hiˆx±?SQõъð?ïøI_Åbu?UjÛe Ô†?NځxÙ-m?UjÛe Ô†?î	{0øÆP?»"ò(¦è?¯hLñO'?»"ò(¦è?íæ@
·"Á?¦Z¹B®É?°Íÿ'´Ýt?¦Z¹B®É?îïû'—}Ç?•'R÷uw8?¡Féؑ?•'R÷uw8AGN3FGL J2107.7-4822@uîâ@1HwÀEéÿãzŽÀ:Ú
'/ðÀ;ª¢år¶¿È¯!²x@d
"Íڔ@°vÿeÑ@¿êÎ+‡ ÑO¿ëyµbÛ¿Ûý裗õ*¿Öû%¢sTXAGNbcu@€ßi­BÃÊPowerLawPMN J2107-4827?ïÿÓ4ùdŽ>öÃýºi‰D>öe•â¦X~>öÃýºi‰D?ïÈ#7ñ¬?'G	º}?{îcþˆ­Í?'G	º}?ïÎ@ÏAàå?xæ,$º4E?xߘ@ÒýÄ?xæ,$º4E?ïûo¼]?,˜µà0Q?CŽ@˃·?,˜µà0Q?ïÿÁA[óy?Þ&¿ÇÇ>ÿ_Wòµ•ô?Þ&¿ÇÇ?îâÉ¥ó;™?¶-D<ã
Á?¡Óe£_ûo?¶-D<ã
Á?ï€ÙA­Òê?Šk²¹Lӝ?É¯žÚh?Šk²¹Lӝ?ïÑèü
0?hÙ5n×c&?w¹øh?hÙ5n×c&AGN3FGL J2108.0+3654@TF= ÿ:À،` &;À9ûì_9K{À;8Ò¯dÝ?Ú£D¤Zú@
ŒnPzÂ?þñæ­j1¿ì¯ižª%¿Ò
ØznÊÓ¿Ò8ÁS-4Ó¿Ýäî–VAGNbcu@±'öE¡ÊÁPowerLawTXS 2106+367?ïýÀ}MÍ?2‡ØŽJ
k?1ÿ#!z#f?2‡ØŽJ
k?‡¯?že¾ûÇÄÍ?ŽRžAûÌ4?že¾ûÇÄÍ?ïá ×ø
?h¸*©Ké8?nüß.ç-¨?h¸*©Ké8?ïÄõŽ³Ê?_w¦¿AÕÖ?}…8ás5?_w¦¿AÕÖ?ïóXRZ‹?XVŠÁª?YO[¹¢?XVŠÁª?íP£Ja<?À¥HŠÍ?·Ízå?¡?À¥HŠÍ?ï²îÕ¾Áz?'ËŽƒ…H?ƒDJ"øë–?'ËŽƒ…H?îœÏ³ÔOÅ?"I!Þ¬[.?¦3ÅN¸§?"I!Þ¬[.AGN3FGL J2108.6-8619@s&¥?À	pÀ=)¿"å­À:¯º¨¦À;Õ"[tšÝ¿ë÷>$þ½
@|É®4[Q?û×à3¿Øm1Vd;¿è—t¡mN¿í§Ðë"6Ë?펨¬S|÷AGNbcu@ÀózáG®PowerLaw1RXS J210959.5-861853?ïú†­>ù ?I¤T¾ ºŒ?EåKM9"É?I¤T¾ ºŒ?ïËoÉ«I?'ôeóòâ?zH3JwÎ?'ôeóòâ?îùþ'7?—'6jdº? `^˜?—'6jdº?ïÿú§"Œ>ͽ8ª>ÅbKìNóK>ͽ8ª?ïç—u@ã?q.b÷ð‰º?hhŠú5¸ä?q.b÷ð‰º?ï-E·³ú³?¯ÎY¨ˆŒæ?šWI¨¤?¯ÎY¨ˆŒæ?íÃ:%Úsî?£k\Çô?±æ.ÐPy?£k\Çô?ïþ½ac¶ø?1¨"{Ôi?$)çÊÉü/?1¨"{ÔiAGN3FGL J2108.6-0250@G±$€	À?"›Ÿ-WQÀ:6û>ÐÀ;á3}]?à{@,Ù@
¡nŠLI°?ÿz 'z?îÖî&
Û¶¿ÑùÚ*Èy¿Ý0°ä+Ž¿ßF³u/NoAGNbll@¬6ÇE8ï5PowerLawTXS 2106-030?ïþD;n@%?,:‡ Tc?+¼I™*?,:‡ Tc?ïƒÖK¦œŒ?šX`"?gŸ?
my¤ï?šX`"?gŸ?ïÒáæ?júMLJ¶<?vñôxß!%?júMLJ¶<?ï±Pq mx?fÞø&wx?ƒ«ã¿Ð?fÞø&wx?ïù±EC^?JqM¶"ŽÔ?I:ê9p?JqM¶"ŽÔ?í"ʑQ?ºÜ:ui0?³_©¿ï~?ºÜ:ui0?ïkHm­«?Œö.ª?'–òMÏf'?Œö.ª?î‡ÊLp?•/£f	?§ƒ[:tB?•/£f	AGN3FGL J2109.1-6638@txYÀe¶=ÀC"ÿ®¡iÀ9‰³Ò*àÀ;ª'	±¿ÔZ䯘ñ@Ô×cL@´ 06ª¿æÀøùÙþ¿Ú"Îl›E¿â;ŒÊº¿à–j»­AGNbcu@ž¤ß;dZPowerLawPKS 2104-668?ïüøL§?4ÿ&a™ëJ?8?-/η?4ÿ&a™ëJ?ïͅ©o?'~s­:?y=+Q`ôx?'~s­:?ïтöXÑ?wc¹;+…?w>"ËXdå?wc¹;+…?ïùœŽ
à?4uó‰ó8Å?IÇPƒOY?4uó‰ó8Å?ïøÜs¡k?JÔ Õ÷™`?LŽ4- Ä¡?JÔ Õ÷™`?îð%(G`¬?¶_£]ý1? ý­{‰õH?¶_£]ý1?ïˆ[Š-–?
à1£,?é>tš‡?
à1£,?瑱l´?wÀiÐkü?…{«öÆú?wÀiÐküAGN3FGL J2110.0+0812@Mş±áÀ9׊Ÿb0À9(µ)B©À;gS˜-ˆÏ?냚þRþ@3N5m=@š)€Výh¿ç˜õªf›j¿ß'<ä{®ç¿ãÐJÝ7ÂÔ¿ì†Ð¯ÝAGNfsrq@•*™1PowerLawPMN J2110+0810?ï°ðxá?´À¹['`?ƒùÃÙfÁ´?´À¹['`?ïEÚxÃ"?¥¿ÞÈ3?—D°éT]s?¥¿ÞÈ3?ëŒëÚ?bR?ªŽéÖ1 B?ÁÌP—v¹?ªŽéÖ1 B?ï}NèÏ?w6-Ãm?>0[JP?w6-Ãm?î¿=>hµ:?£]ãxs?¤,äH\?£]ãxs?ìf	è1?š"`Ó?¼Ï·¸¾wõ?š"`Ó?ê¸&¥"?® NtÖ?Å÷eÁi±?® NtÖ?뙆kê^Ù?¤•v5³¸?Á™æPV"œ?¤•v5³¸AGN3FGL J2110.3-1013@Cè
`:Ó;ÀA·q?Þ<aÀ9™,å;XœÀ;˜£Wˆ}?íjìÖ±@íÌR(—@±íӄø¿âœJ–|-οì‹ßG<™¿ë,•yT¿ïö©¤2-AGNfsrq@x‡<žì¿±PowerLawPKS 2107-105?ïš^2Û?¡˜MA?Ÿ¬´4—º±?¡˜MA?çÂ÷>˜ö?ÉÔ.	cè?ÑÄz'Î?ÉÔ.	cè?î?Ü9"ä‰?šÿ…ì—v?¬<ii…h?šÿ…ì—v?ç
ªIPg2?§u'Ñ®r?Ñê«m_1œ?§u'Ñ®r?ìÝxc
ˆ¼?ºg+»Î*y?¹<écˆ?ºg+»Î*y?Îl|s ¼—?Í{Õ2ác?èdàã7ÐÚ?Í{Õ2ác?ê¥ÄÄ%ðf?²JF«M/»?Åhìïh>i?²JF«M/»?ÅÑý¦á?¦£Çñ à™?ꋹÏ–H?¦£Çñ à™MIXED3FGL J2110.3+3540@Tå€!ùOÀ Éî E>À9­¸¨RšÀ;kŒñëjG?¨—VrxNŽ@çêô€@(WÀi ¿ä¼ó¢	æÅ¿åû§":´Ô¿èþ8
,Ñ¿ïÿv¥NAGNbcu@'ÅquŽ"PowerLawB2 2107+35A?ïìT§w'Õ?f"MC_
?c«XŽW‹H?f"MC_
?…7{±?™"qÔc?Œž¿ßƒ¨?™"qÔc?ïÙÆ8Æ?Œû's¶|?œ¤Ç?Ý1?Œû's¶|?ï¢^›…›Ð?k€Vfèç?‡hY¹Ô#?k€Vfèç?ï{r°²Ì?'¬bh*È?'©áyñ?'¬bh*È?íUiBR¤¬?¼O?¥©¿¤?µTµë³Ÿ?¼O?¥©¿¤?í^)°Aj?¦Jýú;E?µ²|<Ý?¦Jýú;E?ëŠ~µ"ó0?ªY¨?¦h?ÁÖ+t3??ªY¨?¦hAGN3FGL J2111.4+4605@Vy?ò^W¿÷v•âHŠÀ7ÙôŸy­kÀ:ÔàáVǍ@›}¸èi`@©€`7£@EÓ¿b:¿Ôqeóп۔Îs•ùÒ¿ä$Ä
'f¿éÖéë¸í"PSRPSR@'Îq[W>«PLExpCutoffPSR J2111+4606?"ƒ½Ö¾'? Yí"3'?ï[çÁè¿? Yí"3'?¢ø}N¼#þ?»Ã5ØÒ?îÐx+=y?»Ã5ØÒ?ՎÌt,?µ(X•– X?å8™ÿÅój?µ(X•– X?¢Á°\PNQ?ƒ¼{'Ån?îÓäúH¹‹?ƒ¼{'Ån?‡5ÝÈÎ?ŒV=i¹¯?—_'œ?ŒV=i¹¯?ˆiÊwq¡d?¨"±,w?ïžXÖ/÷ê?¨"±,w?Æ.|c‹ð?»o[¾êÀ?êt`ç]?»o[¾êÀ?tWü'¨Tˆ?c£W}ÖG²?ï×Pä±×?c£W}ÖG²PSR3FGL J2112.7+0819@MZqÀ6¼UÀ:OoŸËÀ9‰˜ð&n)À;b8¤Œ;ã¿Á"^¡\@r¸¥š"?ü昛ü ?݋ë¨|'Õ¿ì®w/?j?Å¡(†Sc!¿Ýæ×½
3'AGNbcu@´3UÜÆ?PowerLaw1RXS J211242.5+081831?ïüò$ÂO?dÝ…ˆ"Ø?8oe‰4i?dÝ…ˆ"Ø?ï"d"¨hê?¥Ô}%‡³o?ŠæÛåÅl?¥Ô}%‡³o?ïÅzp^ŒÓ?~³3?}Bdz,ò?~³3?ïýqÎ'?&t£ß3
?7|yžq=>?&t£ß3
?ïý$'ã—?9_Ð"0?6Ûçædh¬?9_Ð"0?î|£?=`;?¶÷žG(]—?¨5Ì	–GN?¶÷žG(]—?ï›i«kG?‡ûh×ßïL?‰%•4öL?‡ûh×ßïL?ïø°pÔ1#?FîzZ…ÐÄ?M>=S:'?FîzZ…ÐÄAGN3FGL J2114.7+3130@S¢åx•À'Äi¿·:"À9ÿôU§ÒBÀ;† Ô÷=º¿úÂc·àV—@Er•É«Z@ʺŸÎ'ô¿á?+¡Ä`m¿íñw³Y¢ø?Ù"V³¸¿ì¸ö´&ãšAGNbcu@"úâëC-PowerLawB2 2112+31?ïà˜¢ú}?t[Wˆ¸Û?ogæ'!K3?t[Wˆ¸Û?ïï Ó/ù?‡0eߔ
ö?~(/•¸B?‡0eߔ
ö?		¥?›
ƒ²>»ƒ?¯Dç|Û°±?›
ƒ²>»ƒ?ïÿØ~lþ—>ïۇ½È¢>óÀë}ÌÇö>ïۇ½È¢?ïĈ2²…?…"Lœ'|­?}»÷ÃÅu?…"Lœ'|­?î©	¨d&Š?·Í‹™A?¥oe|QL]?·Í‹™A?íóêÎÉó?¡­µgwÖ?°`©ˆj?¡­µgwÖ?ïþ'nŸã?01vw-?#®y>ÌÍ?01vw-AGN3FGL J2114.9+5448@WÁûbâ@'ßÕ=4À9Á¸øÚqÑÀ;ÉÜCbU`?ø½üë"£C@·\^¥§Å¿ùÄ™€í¿ÞYÀw÷)忲o¶*ÁA¿Øђ©æBë¿îiYÙÌJØPSRpsr@¨þA:'£LogParabolaPSR J2114+54?çqßOþ'd?ÙXû¦K{?ÑA`Û8?ÙXû¦K{?âÅêÁ"É?֐c±;‡ý?Út*|ÞÖm?֐c±;‡ý?ÙF§¹Ÿ?»
îL›±n?ã\¬v@#1?»
îL›±n?Ùty9t7?Ç*¡iFÀ"?ãEðCcEä?Ç*¡iFÀ"?扊L–þ×?Ú!Z 
?ÒìëfÒR?Ú!Z 
?ÅÖk€›_±?Ð58WE?êŠeÙ(?Ð58WE?ÏكÌJ=]?µŒd©',Ü?è	Ÿíp©?µŒd©',Ü?°â»Ÿ[ƒ?·™@ŒWÔ¸?í㨌YGÍ?·™@ŒWÔ¸MIXED3FGL J2115.4+2933@S'"Àh¡À*™egÊÀ8ÛN?(3üÀ;lw—|?áNø>ѳ"@ʱ…¶Ÿ@û
_d¦¿å•´|ôÈ>¿çæb3Ò¿àÔ¡Vì¿Ü]™j#AGNfsrq@‹'çÕfÏBPowerLawB2 2113+29?ïýËÑéÛë?0>i®œî?1¡nþÒ	Î?0>i®œî?ïƒcCz?ŸáMÚ ÂO?':xï!ƒ?ŸáMÚ ÂO?ïæ8㠊?mª{¿ÃÌ?iÇü9<-Î?mª{¿ÃÌ?ïÀP•CɃ?`²3Þ)¶?×µ?Þ®t?`²3Þ)¶?ïù>zÊæ?K"ìs?K±1x?K"ìs?íÜɌ¦l?·ØRáÖ¢?±³œyÿ?·ØRáÖ¢?ïB9nò¸*?'°IÀ"?—¸Òñ,Á?'°IÀ"?îN;ïè?•úOšz´?«ï;e‡?•úOšz´AGN3FGL J2116.1+3339@Sóˆ` ÒÀ%K@¡À7ôò3Ž£À:Öøp¿…¼?êíª2‰b@AVóרž?þ"ëßâ~:¿Ù@Müì¿à‡Ùí`"ê¿Õßy¬X&÷¿àŸA=%êAGNbll@ž(aaä÷fPowerLawB2 2114+33?ïÿ<ndÛ?kD¯Qò?r<A6?kD¯Qò?﫧ì2™?'6–pîuV?…=÷4éç?'6–pîuV?ïÍK¾"¶?|ÇǺÌ<­?yZ!áá!?|ÇǺÌ<­?ï÷ÌÕ'±—?3LVFÇ»!?PfV:
0Ú?3LVFÇ»!?ïþbHÊt-?*s–¸OrÀ?)Ût9
§?*s–¸OrÀ?îé"bG?³
-ïÂê?§nF
Ž?³
-ïÂê?ïÕΕÇ"?€‹ê™;#?uµqýÖ?€‹ê™;#?ïï{õÙ?T!4ŠK ?`"ûh¿?T!4ŠK AGN3FGL J2118.0-3241@(üT@Éô«ÀEó; g~"À:BÌ}À:æÈ~‰rÛ?ۊÒðÄ@
CùÂ#P'@|#ꬿè­Xíú;g¿è`"·"Ò¿àƒŠÚË#f¿Ùq·z!¦AGNbcu@§1ç»/ìWPowerLawNVSS J211754-324326?ïüÔq±É?I6Vò]?9\q¶Ì¾^?I6Vò]?ïϘó¬`?‰9Wi½@º?xt³yË8D?‰9Wi½@º?ï>ñFÌ®?"P
½ç¸?˜!×(5ø6?"P
½ç¸?ïé@³¤\Á?TÃXž½F?f¿LuÀF»?TÃXž½F?ïëtẀÖ?qæ<¨±sX?d‹f{iÃ?qæ<¨±sX?îùÊ$W?©ÁÐx¨¿? c]²ã—•?©ÁÐx¨¿?ììè2³?«x™¡«­?¸˜¿vÝ]è?«x™¡«­?ïqꆤ§ó?‡°Üöz¦?'¯)³3?‡°Üöz¦AGN3FGL J2118.4+0013@Iû
ÿ±À@Œ@ÃÀ:Œ"\BööÀ;ÓáYKË°¿âM4CÝ@
Ž°?ÿ_@wÏ?4…¿è&Ÿ«Ÿ¿ØÀúýÈÔV¿Íô÷×E)]AGNfsrq@­¬A:'£PowerLawPMN J2118+0013?ïÿ©ä'>ýZ¢fæ?‡Œp>ýZ¢fæ?ﴫѳ%?zÜ%k…›?'Õ†+2Ë?zÜ%k…›?ïæ›OÁÔ?Z=Ì[é*ì?id°Â¡Ãé?Z=Ì[é*ì?ïÿ®Íø	Ö>ôœÀ™\Š>?LiBÕd>ôœÀ™\Š>?ïÿȍ"ù>öA±¡'y>û¹ui)R+>öA±¡'y?îbZˆ•C?¸hú˜^œs?©ÞºWv«Ð?¸hú˜^œs?ï̜ÄØrÙ?w•Ñ·7ý,?y±¯Cs?w•Ñ·7ý,?ïþL©g'?$Ā¤ûÇÚ?+5nW·œ?$Ā¤ûÇÚAGN3FGL J2119.2-3313@'›ÙÀÑÀFê jšÀ9ëãïÿüÀ:ê ;ꊿè6+±<V%@ñ0¯J@ÐÀ¤ ^?îtXûLo£¿Ø	2åk»K¿ì1Vë…ZÙ¿Òàò¹pyAGNbcu@¢Q"¼j~úPowerLawPMN J2118-3316?ïÝòä[N?ƒ¬ƒþ²î?qå
¼Ó?ƒ¬ƒþ²î?ïÐȒU'"?"Â5¬
?w›¶ælÂ1?"Â5¬
?íxô™«že?£
ÒÉД?´8[0}KZ?£
ÒÉД?ïÿj%Z$?%ç"ªß?»X&Dֈ?%ç"ªß?îÙÞ(rmŽ?°+€¶nŠ?¢bxÙ'?°+€¶nŠ?ïYB²õO?¥<Mä-t?"×®I¡V?¥<Mä-t?é5Î@jS[?µVB	¦!?Ë(ÆþV²"?µVB	¦!?ïø¥æ"?LÏu—ü÷?Mhe2IV?LÏu—ü÷AGN3FGL J2121.0+1901@QPàÑnÀ5A/¨;ôÀ8iÎÜq…~À;FŸù/+g?îrIƒ#,ø@J»Þ'òá@DŸWž¢¿à‡àUÆ¿ã0ÅDÿàã'æ&]¿è¹;–
)AGNfsrq@,æšÔ,PowerLawOX 131?ï ç²'u?‡c#sŸp?‡Æi!(Z?‡c#sŸp?ìªj$"'|?¼O>b?º¬®Û[l?¼O>b?ïKLýè+V?"yÞȊ¹?––`IÙÍB?"yÞȊ¹?êÏ0Š‡?¡†cà8à?ÄÃ=×Ñã?¡†cà8à?ì4´ž¶B?¾èdÃNð?¾\[
Mó?¾èdÃNð?àùö_²?ѹ>GîŸ?Þ@›óÞ?ѹ>GîŸ?éüiç^?¶<¸¯=ؙ?È[¸b‡Š?¶<¸¯=ؙ?Ú;@\UZ>?³ŠÚÐJϕ?ââ_ÑÕRá?³ŠÚÐJϕMIXED3FGL J2123.6+0533@Lüa_–hÀ> KŸ:ÃJÀ9í.÷<À;®á?J˜«?ÐU5åGËy@H°Vï¦@`_ÂWÿ¿¸
PíПã¿åk\¨U&׿âGÁÌ#ë©¿â<I}³›4AGNfsrq@–î`ªdÃPowerLawOX 036?ïÿ$¬÷^5?,Üø'¬´?j^nìÔd?,Üø'¬´?ï±p%V?*c÷c]Ï?ƒ£ö±L´?*c÷c]Ï?ïÛPtGá§?r^2 W?rWÅÈÑ\€?r^2 W?ïçWh$_8?I¢ÂõXH?h¨—¡çWÓ?I¢ÂõXH?ïþ÷Äó«?%5R<ê+È? ƒ±¨É]?%5R<ê+È?îd‹•tñÄ?µ³kh3?©·F¦ù»?µ³kh3?ï¡Å;w¿?…Bš·ÚTþ?‡Ž±/Ωæ?…Bš·ÚTþ?ïR'\U¸¼?€—qwñ¼?•­Ôni°—?€—qwñ¼AGN3FGL J2124.7-3358@%ß# îøqÀF¹ÿÅGÀ7õˎß+À;MÀ‡D,€@ªaèÓ>@Käÿ¬ä?õƒ…UE¿¨¨ƒþc¿ÒPòÌ:֖¿ä¨‰{¿ï"å™ç+PSRPSR@'^$Z¬PLExpCutoffPSR J2124-3358?;•­»'¢R?C)óÙñZ?ïüJ3ˆv?C)óÙñZ?ÐS=slÍø?֍ؚ$GÍ?çÖaFI™?֍ؚ$GÍ?¬ÿûg-Ðb?¢‹X폷"?î0I"ú?¢‹X폷"?Y¥ސQÆ?HD$ïkď?ïó-xwú§?HD$ïkď?NR÷.½±?C-œCÛØÂ?ïøkAþŽL?C-œCÛØÂ?ƹ4ÒÎ!>?Ôy2O¢C{?êQ²ËLw°?Ôy2O¢C{?–Ô'M͓F?"ªt¬Qž?ïI[íLÛ6?"ªt¬Qž?1ìy¸6?-'߬isc?ïýÂqÛð?-'߬iscPSR3FGL J2126.5-4605@všßµÝÀFÒf€g™lÀ8Fo?Rü&À;….0Dk?ñÌs)˜U@nšúíœ@¯àÄ¿âúz§]sñ¿çžâ¶:††¿çê^¹ÚèÕ¿ëøSçïÏAGNFSRQ@{8~ùÛ"ÑPowerLawPKS 2123-463?ïûáo=œæ?CÑ<ð?@zCt3zÄ?CÑ<ð?ïÉ{ëDm?'ôÝn!õ?{B
Z"­e?'ôÝn!õ?ïÜFM¨f?ŽŸkóSò?$w1#‰S?ŽŸkóSò?ïøô+œ¢?:mfoÔ?OÜ.|Ì?:mfoÔ?ïúFP=Ò?ILñС¸Ñ?G²ç¥a¸H?ILñС¸Ñ?ï'•ð¥Ë?­Úq¸^i?›
Aú#ܤ?­Úq¸^i?ï,Ã_Cã?"ù$9]SI?šg""‡Œ?"ù$9]SI?ïíŠýÊq?ZWNîb±?bótêØ7y?ZWNîb±AGN3FGL J2126.5-3926@ú'À9@"ÀGÅ 0!0À:^
ÒPšÀ;ç;¥È|?Ýv­©ÏzZ@
eWСm£@ŸÔà—"ì?ëíÏ¥³òû¿á
§ù®­'¿ß¡¶{%Ò¿ïÿuQCr#AGNbcu@˜(:'£PowerLawPMN J2126-3921?ïE'†Tî?®)Á4°d?Ÿ×Mª
ø??®)Á4°d?ïjª¼4VÒ?¦†»Uâý¿?'ª¨yu%¶?¦†»Uâý¿?ë-Ë?©ø¿ž)åñ?×KôÓ¯ž?©ø¿ž)åñ?î;ns%;¤?
Ú·}?¬IËôwÆ?
Ú·}?î¥Rë'é/?§±Ä^™\k?¥ªÑCaÑ?§±Ä^™\k?íîEöâÓ?ÁüŸãŠ©?· ÏÚõå?ÁüŸãŠ©?뱉-p?­eêé¹?ù9ÛKžB?­eêé¹?çUžÅ¨kD?¶UU. Œ?ÑTÂt¯)y?¶UU. ŒAGN3FGL J2127.7+3612@T֟ŸØwüÀ%%ó_ÍTÀ9\M}À;DÈ6eÛ?㛽®CA@¼¿ºÀ…Â?þb±Èd¿Úè—-®¿áDâŒôçë¿Ô©fK
šr¿Þ"%öx†"AGNbll@¥¿û~ÿ—PowerLawB2 2125+35?ïö؀xû?KÝ£ç\—!?RNÿÊëY?KÝ£ç\—!?ïw¿È?óû,4%?'·"ý	?óû,4%?ï½Õ'AÒø?yµÒÉHÛ?€ŠŸm{~?yµÒÉHÛ?ïu¤5à?nñë›9s?'KyG‹ý?nñë›9s?ﭏ:-(?'H³Ö7Uì?"œ1r•~?'H³Ö7Uì?ìg§cS-ò?Â'.çÝ?¼ÂÄåfr?Â'.çÝ?ïTNJÞ?'6‡`
@?•v6¥ôêÐ?'6‡`
@?íœÄhnj?ž•õ•ÛÙa?·Sܹß?ž•õ•ÛÙaAGN3FGL J2129.6-0427@Hu9ÿÖ•ÀBsÇä¡ÖÀ9G¢[	;À;"ËÚ^†?ôß»6¢S|@dëÑëþ@½' Pˆ¿Ø]:vQ¿â©'…UêÿçY¤4ŽcA¿ìŽËj!0ýPSRPSR@sR½<6PowerLawPSR J2129-0429?ß,kgpì@?ËiýXʋC?àiÊLG‰à?ËiýXʋC?ävZ±–)f?ËÍEuß?×JœÓ­3?ËÍEuß?æi¨AAÂ?³å«,HpM?Ó,¯}}ü}?³å«,HpM?ä Úß<Å?¤çGYRN#?Ö¿JA†w?¤çGYRN#?°=Q?†ÕQ?­ˆ̲Q ?íøUØfæ?­ˆ̲Q ?Ð|—rDb}?Ìý
À€ì­?çÁ´FÝÎÂ?Ìý
À€ì­?ľ$.n¹'?³†½ÑŠ¶M?êÐvôdQŸ?³†½ÑŠ¶M?ÇjŸj,ÞI?£Dô!ö+?ê%X%tÈn?£Dô!ö+MIXED3FGL J2130.8-2745@3ÿV_ˆ%ÔÀFéaÀxiÀ9àwŸsÎ.À;¾:bÒ]?ðÍB"xm@
£*ƒ6UÒ?û-_ÿÄñ·?ï:ÀÎÅS?íãqàÃr¿Ö‰í›	Â]¿áoxæñ'AGNbll@±'ñ©ûçPowerLawRBS 1751?ïØ©¨
-n?ƒPæwÔ´?s«,¸?ƒPæwÔ´?íZEg#‹Ü?¾,B#ø?µ-ÔÅ+Ó?¾,B#ø?îڀ™îS/?—bÙF¶Pg?¢Wö]«1?—bÙF¶Pg?ëú~âë¿?£@{ŽIaü?À€tQ?£@{ŽIaü?ïÔã™da÷?z•3^¡Rû?uŽ3mklx?z•3^¡Rû?êppÄ÷—?É.P²?Æ><ï¨!¥?É.P²?íÆEæ?¢ ŸG[ô?±Ï5ÐÏïJ?¢ ŸG[ô?æ€AÏ6ñ?¼Qv¤ÖR?Òÿ}âa'?¼Qv¤ÖRAGN3FGL J2131.5-0915@Eòp_äl&ÀCÕQßƤ•À9^YûIÀ;…¸¿Þ¨?Ø´öp£ðÏ@߂ÃiKÉ@1ÿ¦™¿ÜVÝaÅlÜ¿ç€À¶F¬¿ÛOt2$¿ÆW†àÀ†AGNbll@ uA [ÀPowerLawRBS 1752?ïþc.÷?+<6¯š?)ÎîwÂjî?+<6¯š?ﴖ+W³?"[ñÙ¦ÃÜ?'ÚuH€É%?"[ñÙ¦ÃÜ?ïß¼U¹Î?há«×4è?p~!Ê$XÔ?há«×4è?ïñ%Ìî/É?DAÓÁ˜]•?]´f¤.M?DAÓÁ˜]•?ïûi˜JA?Cvׅ2
?BYŸètÇ%?Cvׅ2
?î³ÃO[Ä?µN¢‹—?¤ÃˏB†?µN¢‹—?ïše¸±À?†	Éj]:?‰fºJôWò?†	Éj]:?ï¦Å©S1?wôT^€"?†xœŠk¨?wôT^€"AGN3FGL J2131.8-2516@7‹yœÝòÀF½aßîèÀ:C(ǀÀ;×>â"Þo¿÷Æ<lí¿@´Ô©˜@ÿÿ&§¿à¤\—ÊP`¿Ú§Û%Õý¿â"Ò«Å&v¿Ü.ÛHP7AGNbll@¤…)^ž	PowerLawRBS 1755?ïÿ
Í
`?¡àE¢?¦YÚûö·?¡àE¢?ï×K[¹J?†W®s¸Œã?tZ8KD"Ï?†W®s¸Œã?ïÍ—ãzÓ?vþ«²™òd?y|´£®"?vþ«²™òd?ïÿá"hþ>íVHL•>îáJ#rÔ>íVHL•?ïýá)¦«?2([8°?0ö³Oï=ö?2([8°?ïc$^ü\)?Ÿ"zšó-V?"›t tzâ?Ÿ"zšó-V?ïe
b¾?,£X&‹?"^]uVE?,£X&‹?ïýØcêò8?/¾c¿« '?1<â[ÖWY?/¾c¿« 'AGN3FGL J2132.4-5420@u]8À>-ÀFqEÄÁfÀ9Gíf H
À;·¢šÊB¿ë¾É e@d¥‰çÊÕ@X`"?h¿åÊv''²¿é´ìӟÇ(¿á†1/D^¿ëˆÎé¿7AGNbcu@~'»dZ¬PowerLawPMN J2132-5420?ïþŸæè%?&Й?#4?&Ÿ}«Ò?&Й?#4?ïÉߑ9gš?'­'5Qd"?{7}i;?'­'5Qd"?Nvì­?÷¶Ya?‰,bDÔ×?÷¶Ya?ïÿ¥ˆ>ú‹3´¿8/?¾(UlU†>ú‹3´¿8/?ïÿ'>‰'±?ô}îL?phtp	?ô}îL?ï7ª‰´|Ò?¯.H¯©6?™
®Ç¸—µ?¯.H¯©6?ïÂ
Àg?ˆ}¥–SÉ>?ˆžº(?ˆ}¥–SÉ>?ïüî'DŒ?2@¬éd!?8‹oÌ&͒?2@¬éd!AGN3FGL J2133.3+2533@Sy?ò^WÀ2ñ1Àll:À:IÑqw<À;¥É¤úì¿ìþgƒ¿4*@
Ÿ3«S*t@çU ›¿ìxÛ¢S¿×gb!sK¿Óþ;ĕ¾¿ãÞ
ùÇñ`AGNbcu@®ˆ‡»/ìWPowerLaw87GB 213100.1+251534?ïþ´¬M.?'A©0õ8?$µ>—'?'A©0õ8?ï±ç_¹è³?"ÄBk‰?ƒ†(<a?"ÄBk‰?ïà¿(Û|¤?lõÊúgF?o@ÖêÉì)?lõÊúgF?ïþô¨ÅÜ?Z¢ÔÅ? µso‹‹?Z¢ÔÅ?ïúíc	(Œ?ErZ<·}?DJtn&¶Î?ErZ<·}?îÅk!¿ ó?³êåþ±?£©MäðÒ?³êåþ±?ïÃ>7ëv(?~«g¾%x3?~`ãéø˜_?~«g¾%x3?ïôÌÏÀ¶Ù?Pú9`)¦?Vf`o9?Pú9`)¦AGN3FGL J2133.8+6648@ZLhß½jY@&5Á'ì¯À8öüšòÀ;Fçž	jãÀ»zgODŒ@·5Œ©Ç@ŸMÀ¨&O¿çv\{è¿åŠÝì&PÄ¿ÅõJç¦9¿Þu&HÐ9¥AGNbcu@¤ªv¡aä÷PowerLawNVSS J213349+664706?ïÿÎä¡w+>ñp¸Þ¢>>ønÍZÐ>ñp¸Þ¢>?ï×4v̇z?…
be¼!£?teÄ©Švë?…
be¼!£?ïñ‰5¯uŠ?`@
ÂÑmf?\픮Ó[•?`@
ÂÑmf?ïÿÿés_>p/pÀöp>f€kØkE>p/pÀöp?ïÿÀjîD>ÿ²'2獫>ÿÊïê½:µ>ÿ²'2獫?ïBJÚ2ª¼?¢æÃ'Žc?—¶¤À‰ày?¢æÃ'Žc?ïì.èSn›?s•YâØ#ƒ?cÑÆ®mA?s•YâØ#ƒ?ïÿþ¹­f>©¶ä1*ä‡>¤r-µÊ°­>©¶ä1*ä‡AGN3FGL J2134.1-0152@J3lÿݛQÀB>Ÿ¾vÉÀ9ÂzcÀ;‰Ê)"]È?êåúr¹9@_Ə@¨õ (š¿Ûk–/§¿åB¿©^ð¿á*èàÃh¿éžäq%©AGNbll@-žÑ·PowerLawPKS 2131-021?ïþ	áf7?,†Œ`Eñï?/o®ð¿â3?,†Œ`Eñï?ïš>Lš?ŸÓÜÐ>á?‰°z¶Éc?ŸÓÜÐ>á?ïÂÉ*xF?x&Z©º1?~þ›q£ô?x&Z©º1?ïíjCÀŸ?CÇkÚð;Ï?b•»ýhiU?CÇkÚð;Ï?ïüéœÞ"î?;q$!–ú?8³Fˆ-?;q$!–ú?în.•?ºd_2%Ó?©	?·?ºd_2%Ó?î(~|
Š?¡ÖCÃúZ?­x©÷%_?¡ÖCÃúZ?ïÌ'¦a9?iµ7a›ª?yìv& U?iµ7a›ªAGN3FGL J2135.3-5008@u·©³únÀG1Kÿ²Ó'À9&*·c®üÀ;ti;'§?å¦Qs˜±›@/Á™gð@Â7r@º¿â]Pì4Nſ磷쯯õ¿æ
fyG¿î97²ÚïaAGNfsrq@‰˜G¡8PowerLawPMN J2135-5006?ï»[ãÝ?ƒÄŒ€¼0þ?)>â̧?ƒÄŒ€¼0þ?ï"Õĺ|
?–.QEC¶K?ŠÊŽßm€?–.QEC¶K?ïAÁÁUö?`K¡}Ä?žÇÇÕA;?`K¡}Ä?î{_±¸ÁŸ?‡‡{<"ä\?¨Jè¿i?‡‡{<"ä\?ï¦y€i?°Ðá½j?†a½ÕÑÝ?°Ðá½j?ë»5pOHh?ÂõqHdI?Á*>ÂÞa?ÂõqHdI?앞"üj…?«€*6Œ?»Sè«Õ?«€*6Œ?巟F+ÞU?³"ÝЧ¹?ԐÁs¨CV?³"ÝЧ¹AGN3FGL J2139.4-4235@vdڀIf{ÀH)οìºÀ8àÇU"‡À:ýÂÅ+?öùŠ¨ex@ðÀêÁTt?þ.` ©®:¿ÚÚ$¿à‰ñ]]%¿âª-qI¼¿å¹·©AGNbll@†éÏv_Ø®LogParabolaMH 2136-428?ïÿ%,4fd?$æ ×\͏?Z|Q¬Ç.?$æ ×\͏?ï¸Èê¦7É?"S÷Ú߸v?ÍÅSZgÏ?"S÷Ú߸v?ïŽ#YKuÊ?‡¸nÙÂø?Œw)°')o?‡¸nÙÂø?ï™ËSX 3?pcnxOeM?‰+©çg?pcnxOeM?ïý­ø˛?>üÀEô#?2@َ^´?>üÀEô#?î­ôѽfA?·®µŸ/?¥ ²æ½Pè?·®µŸ/?ïw­h®j6?'q-m52s?'
Rññ1?'q-m52s?îút䔥Ð?D4öuƒ? X±¶µ¢þ?D4öuƒAGN3FGL J2140.0+4715@W(üà%o%À-J?¿2°À8~&vŒNWÀ;9ÕÓ܋‡@ÆèVÁ@
b)Üó5—?÷òˆæüy?ƒMc¤ÙØh¿ßæ碈x¿éÀ9ÖæV6¿ïÿߓpW"PSRPSR@‹¿ùrGEPLExpCutoffLAT PSR J2139+4716?V˜ã]ªM?i[‰/ê­?ïôý³I˜û?i[‰/ê­?ªbM^òž?Ãé‹e_'q?îYÛ*U
–?Ãé‹e_'q?¥¬R#¦\Ò?˜â—yëS?î¥:ݪS?˜â—yëS?wµD®ÒY2?`¥VŸ÷'?ïЕvÊ6Å?`¥VŸ÷'?X$V©õ§?dnuP$ŠÃ?ïóíùÿF-?dnuP$ŠÃ?Ž£
>nç?­\ÆÄ9?ï…Ét?­\ÆÄ9?Œò¤€[Ê?‡bi¿|Ñ9?ïŒ5mþ"Í?‡bi¿|Ñ9??•­Y`þ?0ëx)èO?ïü
JI?0ëx)èOPSR3FGL J2141.6-6412@t‰¢ß"xîÀE!'	±À8úÙ*© öÀ;¦þÍÐØË?ñ€=û8E@"ž­Õ'@ö?[4¯¿âuöÉk¿ço7HŸ3À¿ç>‹Q¾tÖ¿ïûdÒÁAGNbcu@–\(öPowerLawPMN J2141-6411?ïêõÞÇ?r·EC±{¨?eì
eð°é?r·EC±{¨?ïÇÈüˆ§.?'ôŠoÉÖ<?|°­©?'ôŠoÉÖ<?ñÝÜ?ŽÅ´Ò™¨?Kã|?ŽÅ´Ò™¨?ïÛîï(	?VÚ®"†»²?rˆ}{˜?VÚ®"†»²?ïõy(àÉÚ?[âߛùö?U
®Qª??[âߛùö?îøí53NÈ?´Û¾X5? q,¯^Èz?´Û¾X5?ïâ7uÀª?•‹¿¤5Î?œã¹
h²É?•‹¿¤5Î?·(²?™Púë'h?ŒùÓßôCu?™Púë'hAGN3FGL J2141.7-3734@|XüŸ£ÀH…ÅŸ±áÀ9º;Ú¡¡¦À;ÂÊ榓¿Ó$šß>êL@ÿ<ú\R@»e€À¿á·b¾w¿í$FŐk¿Øm<7­…#¿çƒÔ¤˜·XAGNfsrq@€¢ŽŸj"óPowerLawPKS 2138-377?ïÿÎ8Kº?«Ž½Üõü>øãèIA¼¸?«Ž½Üõü?ïÎ"Ô å9?'~2I¤í?x½–ŠãY?'~2I¤í?ïÝ­¬îWƒ?v…YT/Ü)?q))åBV?v…YT/Ü)?ïþL
õŒ	?ÈΞ6Ë/?+?9Öl?ÈΞ6Ë/?ïÿã\}¦Á>ïڂ½>ÙÔ>죞ú&Y>ïڂ½>ÙÔ?ïN†Épb?¦âä¾Àv{?–/&Û¢WÍ?¦âä¾Àv{?ï¿&
'RL?€uÉ«9:?€6|§e"?€uÉ«9:?ï÷îƒÖ¹¶?E¿D?Ôí?P"øN³k:?E¿D?ÔíAGN3FGL J2142.2-2546@7œà`'ˆÀGòˆÀ-'À:õÊdÀ;ÎþV²"<?âþŒ2'ð_@ªÅ[>j@ىÆã¿àÙ24Z¦¿áø'ÕE¿â@ª½áÕü¿ïþ½FSþAGNbcu@'€âe+ÔPowerLawPMN J2142-2551?ïæHÁöì?lh¤˜ËõT?i䷍t?lh¤˜ËõT?ï¦Çæš9Ž?"-i6þ®l?†NO"Ț?"-i6þ®l?î;†`NA?™H.0Ù«q?§ìG—gf÷?™H.0Ù«q?ï)ºÓ>ñ?}<?+{H?žÈ£àSï?}<?+{H?ï£Âà9ç?ˆD;+Ý?‡Gøew–?ˆD;+Ý?îP^'¨*ù?²Õv§¨8?ªúèh?²Õv§¨8?í_I½Ÿn?£•Â#ìè?µ²Nfv?£•Â#ìè?ê{EõÇ[¸?¬ÜzŸu?Æè(â'?¬ÜzŸuAGN3FGL J2143.1-3928@´j¿f‡ÉÀH¡à f§ÕÀ9å)*›´ýÀ;¼÷üü??Ð9å©èqC@¾9Èxª6@•p@"Õg¿ãù/±¾¿ãSßÁy»¿ã_Ø{4\\¿Ê´ûÀ¾2AGNbll@ YK]ÌcñPowerLawPMN J2143-3929?îT`.éÍd?Ì;ò¨L~?ª¹ýöÞÂ?Ì;ò¨L~?ïÚʬ6)]?‡º`	%?rš©úèÑ?‡º`	%?ï¨}Psñû?Œí"Î_j?…à«ã%?Œí"Î_j?ïúnÏÍ?15NnÐï?FEøäLM]?15NnÐï?ïý54a¨ß?O!%~€<?6V[Ǝ^9?O!%~€<?ïdJÎ
Q?¦'œtÒ?"v¦95î?¦'œtÒ?襁ë8?ŠËõñ»
?…R{Òþ"?ŠËõñ»
?ï×ÒPÖm?iž¤@O?tv–¶˜‰u?iž¤@OAGN3FGL J2143.5+1744@R~_ìÏ¢À:›?Œ
À7ykˆWÀ;™À0X?õ'–‹SH@TI,į@Ò"¡!¿ã·+À^f¿çš+FC ¿è·¾-‰¿èќüê:¶AGNfsrq@t1HýŸÓoLogParabolaOX 169?ïü"ò:Åy?6k
u¿í?;`lˆ¼?6k
u¿í?ï²÷#&e?–o…/:']?ƒ|Â4v¶â?–o…/:']?ïZ[È Ë?Žk­?l;7?"´†åî§?Žk­?l;7?ïظ <mf?ZI¹Ê]B?s£¯Ä<©(?ZI¹Ê]B?ïôÙO€à?Vo§v
M?VMa=wѾ?Vo§v
M?î†Òþو?ºýkT{œ?§'О²?ºýkT{œ?ïaìÉíIo?'Ëé8m?"Âf»wš(?'Ëé8m?ï™rþáX0?}€A	t?‰£@Kæ?}€A	tAGN3FGL J2144.2+3132@T¥µà!=gÀ0Kæÿ}úÀ9©°â‹zóÀ;¡­SŠÁ?³ð˜-›µ!@A]Û}i¸@å¾@Q¿æT-';¿Z¿èL®ITè¿àvÒ&î_¿ØýNʾUAGNbcu@Ù†sBîPowerLawMG3 J214415+3132?ïÿ+-͐?WShÒ»E?š> 	¸?WShÒ»E?ï¡óø,Cw?›-cv?‡ƒç0²B?›-cv?ïèý²Ì"?Wܑ–`ï?gM'4*?Wܑ–`ï?ïòJï¬9ž?BÒ>sk™?[j ކƒs?BÒ>sk™?ïûËs9K?BwEÕ«¯*?@Ò2Šœ#ˆ?BwEÕ«¯*?îc})‡ä?¸[ðl&SX?©È.¯OÂ?¸[ðl&SX?ï«Að˜âm?"<ûtBê?…/ƒÖWÈ»?"<ûtBê?ï…úƆž?糍 Žï?ŽyÜÈy?糍 ŽïAGN3FGL J2144.9-3356@&ó7z>ŠÀHÍ«ÿÍ«À8÷¨§b°À;¸£J"?ça{aŽÿü@f2R7°@\–Þ²}¿Ú‹¨-¡¿åŒv¢¾¿å•GÄø¿è}
xAGNfsrq@‡‹<w¯dPowerLawPMN J2145-3357?ïÿ&ÛOá.?n-{¦.d?$˜)›ÉŽ?n-{¦.d?ïÖÀ36c>?Í—ìü?tŸæ…´Ÿ?Í—ìü?ï©ñ¢çm"?×$Øêè?…ƒ—;ÕÊö?×$Øêè?ïú
ôbN?.÷ù¯i+?G×ôČ®?.÷ù¯i+?ïþ‡ Ùåö?-J–¬}x?'…óºßÂ;?-J–¬}x?ïcÞ`6æ5?¤Y¿˜i•[?""3þJ£[?¤Y¿˜i•[?î­B³%SC?ž[g¡þ+º?¥+ÔËÒ?ž[g¡þ+º?ïïÅ6ø±ú?RNÑÀðª0?`:É"Êå?RNÑÀðª0AGN3FGL J2145.7+0717@OÄ"}À@µt@C¼îÀ9¢ÓßÅpÀ;‹N[­¥ÀÀ'(–ÍŒ@—f´=@@m`€žK¿êö¼»:[Ï¿æõ;4A¿å}©gå9¿Ì#â.‰AGNbll@ƒ£«jçÕgPowerLawMS 2143.4+0704?ïþ­ bé?(4lW&Pê?%-ý–å©?(4lW&Pê?ïÀ€jÀà}?'B}	2\?¿Ê¸Lñv?'B}	2\?ルÄ?h(?tüÎ7%6?€YŽ÷-Ý?tüÎ7%6?ïÿÿ€¤x>¨žš]OÂ>žì¡:™˜á>¨žš]OÂ?ïúI¼ÙÜø?PŒMà™l}?FÙž˜<š?PŒMà™l}?îÄ(íù±÷?·0^ªåw?£½q$°c‹?·0^ªåw?ï(Td}¥j?•Y°û8?šõsk#èÒ?•Y°û8?ïÿß%¹^>öïáúîÄ>ðyϚ1Àµ>öïáúîÄAGN3FGL J2146.6-1344@DT—b%ÀF|ŸïôðÀ9sñidHÀ;t•?ñþIQW¶u@þ¹+ZKÑ?ú}ÿµ,r?ï°'D"?ߦW{¯\¿ØÒùmzèæ¿ÒýGbƒò'AGNbll@±pÏß;dZPowerLawNVSS J214637-134359?ï'óÁòíã?…UÀð®?‹ƒŠ#¿T?…UÀð®?ïN…jsÍh?¡{æöÜ¥9?–/R®¶ø?¡{æöÜ¥9?î¿YOã©C?– ãà›¨ì?¤
jÿ1¶Í?– ãà›¨ì?îv½`
?êºQ'Ãq?¨")þb8]?êºQ'Ãq?ﺉ˜/?—lÊU9?è®ßäÈ?—lÊU9?í¨؝v¯?¶ï´çÕq?²¿É9Êp	?¶ï´çÕq?첛âãÔ?©£IóH?¹êk èá^?©£IóH?ì%~+vrÅ?¯Ù¾²3›?¾Ô¤LiÕ?¯Ù¾²3›AGN3FGL J2146.7-1527@C:\?›÷BÀFØäÀ™,À9åVI¸±À;µ5õ…R»?×¹¬%¯´[@Éª@«À#Ç¿ßíÔߟ¿è¾Zâ,c¿êaJ"wbQ¿ÌO¿iüŒÈAGNfsrq@‰šÅoPowerLawPKS 2143-156?ïþݲ¥?(:vaóÈ_?"/§èïVB?(:vaóÈ_?ïӎ—Zv?€´¿ŽÅ†?v8´R0½ ?€´¿ŽÅ†?ïŸ)jKg ?…@ãëj?ˆ5¥i¶›ì?…@ãëj?ïöÑV…ƒô??L¦á±(?R]Spª??L¦á±(?ïüë$?".?@œžl»?8¦ßØ$ï?@œžl»?ï1[î¤t$?¥èLA:?™Ô'&J}?¥èLA:?î¯÷€™\L?™ì³VŠúe?¥‡öj;C?™ì³VŠúe?ï«Oäf=ï?}ý@IԄÜ?…,æp"D?}ý@IԄÜAGN3FGL J2147.2+0929@PsìZþÀ@#%¿­)™À8·	)7À;?ä^¹É»?ö‡¢äß@±·Å(¾@µƒ.ž#¿áh¯¶ˆà¿è‹A".¯¿èn~K=Ë¿é}ÆTb­ÊAGNFSRQ@vÞx"LogParabolaPKS 2144+092?ïü0
¹Ò?8؃=Ç??^~iS2?8؃=Ç?ï"s/€(ã?¬&/d} B?Žã4Ç»b?¬&/d} B?ï›D× ef?€;é­[¬õ?‰.Ê
—Ò¡?€;é­[¬õ?ïôQîV¬¬?@mýöÈ?W\#µ›f¦?@mýöÈ?ïö¢V+°³?QQbÖ1x?R»S°Ýª)?QQbÖ1x?îÄ¥x…?³•_-1ó?£µ®w®ô?³•_-1ó?ïZÞ ‰ÍÊ?"æO	:Õ?"¤+ò5âÇ?"æO	:Õ?ïëìoª\à?ZG‰
9³?db·™?ZG‰
9³AGN3FGL J2147.3-7536@s¼®_ú;›ÀBD-ó»NÀ7[ðEwÙUÀ;/†è¼í\?ø˜‡Ô3s@Û6"Q@rÑÊãh›¿ã†ž%€©D¿æ销w
¿èÝz!·¾¿é@«}‹ŠÒAGNFSRQ@riÒòäLogParabolaPKS 2142-75?ïî®åAk?bŒŽ|q?aQä8û$s?bŒŽ|q?ïÍ¿ˆìx9?–CDH:s?y ;k‡SÄ?–CDH:s?ï¿àw›å?•\.j€å?èê-Ka?•\.j€å?ïÿ6ÊuO?
—x%ù5ä?&¹¿c~H?
—x%ù5ä?ïîqtۗ?d{ÁñÂD?aŽùyFq?d{ÁñÂD?ï&°K•]?³È^Yã?œÛ)ÿ$ZJ?³È^Yã?ïDc³â#?'´Ô<ë‰?—nS‰ƒ»¦?'´Ô<ë‰?ïÿMçÙ1y?¹0M?éÈ?CöúT"?¹0M?éÈAGN3FGL J2149.6+1915@Rœz?̞ªÀ:
Û L¦¢À9VÆu'ÊÀ;sCWm¥?c©te%_@Sz'î.Ç@Œ' ;¿å
ª
7ԋ¿çE¹*-¦¿ç›@'{Ï¿ïÿîpǤ€AGNbcu@…ñÙ‡+PowerLawTXS 2147+191?ïüÁ¸'Ï?JDCJ*?9ò<zªBc?JDCJ*?ï¼1ªO§ç?"&À¨	œ?€ó•f>°b?"&À¨	œ?ïRðr™O?¤îJ?D?•¡ñ¥öÔp?¤îJ?D?ï÷Êéë
!?6Lc0Î5š?Pj+¥ô¾}?6Lc0Î5š?ïþꜟ/?,"Þ¸¢%?!V4NcK?,"Þ¸¢%?îÉpz)O?·vC§jU?£hø]'"?·vC§jU?ï¢â	8Ҟ?…pdŽlaJ?‡G}¿‰È_?…pdŽlaJ?ïñ|~¥?o}/Áfx?~'A²"Ñ{?o}/ÁfxAGN3FGL J2149.7+0323@NFâ?û˜'ÀBQ,_Ú[+À9˜ÛÈRéÀ;©¼®q—ó¿Ö s8ז@ÖJHùn@4ƒPþ¿ä{Ÿá1]Æ¿Þsñƒ)Y"¿álš¨7l(¿è|/՟sAGNbll@—ëd÷eý‹PowerLawPKS B2147+031?ïþ@¨Õ»?E¤Ð
@þ?+õ}Buà?E¤Ð
@þ?בּ5¹í™?¥ÈŠ+"7Ã?"Ó²'"™¥?¥ÈŠ+"7Ã?ïäøD÷?qÙÆ-lb?krÙE?qÙÆ-lb?ïú,q֏¢?27VÏÈKæ?GN7»M2?27VÏÈKæ?ïý­2uH?/Œœ³t†«?2—>uè?/Œœ³t†«?î³êäB'Õ?´·¡¯w-\?¤ÁQ¿Fn¨?´·¡¯w-\?€L­?´¨Ò~©?‰Ý_÷Ih£?´¨Ò~©?ïÆÚl?Ø?pi'+Àv?|'ÉëvÔ?pi'+ÀvAGN3FGL J2150.2-1411@DMþ_ìÏ¢ÀFú?Ï"èÀ9ÉΠ£¢À;‡ìZ0Íþ¿ó9‰®¿ñr@Â}'Þ[?ýB"!=ƒ¿ãYß­5i¿âÂ:Ƌ¦M¿ÌZMN¿ð¿â‹t™É®úAGNbll@°»À6ãPowerLawTXS 2147-144?ïÿvÇve|?
ä>£Åä?'BèíÄ?
ä>£Åä?ïË·«bð?»ë.?z$u3íp?»ë.?ïìՈTš.?n¡ÕìEäí?c*wÆâ²O?n¡ÕìEäí?ïÿé	Ìæ>âÿðÿÒi>æö
é•>âÿðÿÒi?ïÿ^OÞ?Í3ÆGIÛ??0"¢?Í3ÆGIÛ?ïAÌvѯ?¦%ÿ¯R\|?—Æq>Ê?¦%ÿ¯R\|?ïݖ©Ø´•?vÏDZ‹"?q4«(C]P?vÏDZ‹"?ïÿYÌúïö?ðN/jò?ÆZ{ñ³ˆ?ðN/jòAGN3FGL J2151.6-2744@5PÆ3¡îÀI*èà(Ê$À:'e"'ÒÀ;Ë5™?Ç?Û/ú?\ó\@/‡­@Z€a¿˜"³ƒ´o¿êÂ#ë0¿é­"b€~¿äÔ%¥<KFAGNfsrq@†}"K3ÛPowerLawPMN J2151-2742?ïýÅä-ð?6_ü…M•?1ÐÝtÓEi?6_ü…M•?ïÂy'oS?"ýOžM•?~ùÃ1¹Òœ?"ýOžM•?ïK+0§µ?ŽÖw‹öÅy?–œ:Z¥Z?ŽÖw‹öÅy?ï²Ìå+ö?gxÕ™@?ƒLƞ\¼a?gxÕ™@?ïø³l3?RÌ]fçƒp?M3ùëD<ó?RÌ]fçƒp?îóâšO!?¨"œ4Á/? ÁÞŠô?¨"œ4Á/?íê=>¶p?¡©e"EYŽ?°®
½Ð?¡©e"EYŽ?íXÄ~cw
?£	—`1ؐ?µ9Ü,yž?£	—`1ؐAGN3FGL J2151.8-3025@1!Ef­ÀI`Æ báwÀ8>ŸªÀ;cá6]E?üó¥&@"¬Âc¿@	Eç#»¿çŽ:¼z«S¿íÒ_³Ä¾¿ï+¢^Ô¿ïç®ÀGXYAGNfsrq@k6÷ãÑÌLogParabolaPKS 2149-306?ïói.ËM#?X¦Š7åÁ.?Y-¢Xç™?X¦Š7åÁ.?ïÅç©$¯•?‹Š¼+Ÿ(?}+Q{iv?‹Š¼+Ÿ(?êäÃc®?¯oœqÅ}?ÄlòsÇÅH?¯oœqÅ}?ïÂɜIU?vyÈá`M¸?ŒMœ]FÂ?vyÈá`M¸?ïäH™ÌÅ@?vIë(¨ûÂ?k·fJ˜Ï?vIë(¨ûÂ?ç?§&ßXcÆ?œì	w#Ø4?§&ßXcÆ?ìtެѸM?­8õb‡-?¼Y
™r=›?­8õb‡-?ï	aÀ0ԁ?•$ßµ,>?žÓÇû=ë?•$ßµ,>AGN3FGL J2152.4+1735@RidÜY2À;±< BÀ:"曪ëÑÀ;Ï"‰G<?Óuö
°9;@LxiOò@i3ˆf¿ìn'yÂc½¿Ò¨-}‰¿×'e/뼿çÎM¸<yAGNbll@¨^he"¯OPowerLawS3 2150+17?ïýSväQ½?3´¥Yӕ"?5dHZšŽq?3´¥Yӕ"?ï‹FÖºH?œ¬>­,!?—#pé?œ¬>­,!?ïÏòÓ`~Š?sS•£rºÍ?x–`>Û
?sS•£rºÍ?ï;^;…ÎG?}·˜2¦?˜"8'µÓ ?}·˜2¦?ï÷hÂ6Eâ?N"µjÖfå?Q.{‹5+?N"µjÖfå?ëà¯V*•;?Ã0\áØM?À}B§U«?Ã0\áØM?ï‹Ød@Øt?ˆ4Y¿]$S?	æå{-?ˆ4Y¿]$S?ê
¶1)î'?³K»^H1]?ÇÉ';XE¼?³K»^H1]AGN3FGL J2152.9-0045@Lw©Àª€ÀCÞÆ_ËA²À:I´+'À;ªÕ¥¹cÀdfÇ_Oœ@=½O?ÿ)"_è¿ê¿«4²ËU¿¯anAž}¿èòÖ¹¾0?Ñ]²eöÝuAGNbll@¬¥•ÜÆ?PowerLawRBS 1792?ïã~IS}x?£eN¬i´?l¶š¤'?£eN¬i´?ïËöXm;?"æ[µÊq?zô×8þ¨?"æ[µÊq?ïRwÃ?I=E6¿%?•±½O®?I=E6¿%?ïÿÿú3Z>p¹HOíš>œCpÎ'è>p¹HOíš?ïé3õGñ?g Æx瞽?fÌ
dæ«?g Æx瞽?îÑw£ç?¶ñ]¼"úd?¢èŽ_¥˜?¶ñ]¼"úd?îM¸‰¸•?žÀ·£ll•?«/Du¬¨¶?žÀ·£ll•?ïÿÍÓËD?²˜FÎ/V>ùq¦DÇ?²˜FÎ/VAGN3FGL J2154.0-1137@F>T2TçÀFÔÓßæ…À9:̎¹kÇÀ;ª¬ê¯5ã?î"Uk±Ô@}Ísí@é(€&ÖÙ¿â@4XLGV¿èO'²v¿çƒÉü¿ïÿíÊ"EAGNfsrq@';°U2a|PowerLawPMN J2153-1136?ïý
Ùÿ² ?D°ä')Ê,?7'0¬×¢0?D°ä')Ê,?«ô?'N»Zü©H?‡š‡DŽm?'N»Zü©H?ï.ó€ô9×?'},t©Õ?š!Þ	),?'},t©Õ?ï+³êþ'?vOqJL¬º?š‰'¡å«\?vOqJL¬º?ïþ<Öõðˆ?4*Ì$?,2nî$é?4*Ì$?îVÚº¡&+?°xmýÛùÁ?ª'TW¥kO?°xmýÛùÁ?ïLU5Uø?''‡ûŽ5 ?–u\þ|ªó?''‡ûŽ5 ?ìk'–Fÿ?£{Þ°•'µ?¿¦ÃMÈ
?£{Þ°•'µAGN3FGL J2156.0+1818@Rº6ŸÏ=ÀÀ;Ê	 '²À9ôW(ÛÁÀ;š}=B€®?Ç`d×ù"C@¸]?÷î?þ `"=µ?ïüà*D«¿ãÿl(¿‰¿ÓäŒ&iv;¿ãÓ7m©"AGNbcu@«ÅÖ8†PowerLawRX J2156.0+1818?ïÿrͳ¢?
Ö¾ˆûÚ?¦b–p ?
Ö¾ˆûÚ?ïÁÇWå?‹°ëX–)?TdPJ'?‹°ëX–)?ïà´÷ª,J?l`Ü09{?oKM"¥ï?l`Ü09{?ïê6àÅZÆ?LRqßĒž?eÉêŠ?LRqßĒž?ïÿ*'	cg?­øfôÅ?­ÞàÄËJ?­øfôÅ?î±
ØAj?¶Rß	¶?¤ï"x€
d?¶Rß	¶?ïÇJÔø?{ÿ©y¦¬?|ZýU­º?{ÿ©y¦¬?ï¤eÈ,?v_ƒ]îùÃ?†æ¸ÄÉ?v_ƒ]îùÃAGN3FGL J2156.9-0855@H.­@?‹0ÀF HtäÀ:t䝣êUÀ;Æ£iüóÜ?ÁÜ#¾r@M¯gQî?þm'Ԇª?ïñ½øÒì?ë£`Æ>F¿è'ßSª¿°¶¤cC"AGNbll@¥ß7eýŠÛPowerLawFIRST J215650.3-085535?ïü·•ÐXÀ?Aö—?aÉ?:CPË?Aö—?aÉ?ï¼9ülY?©ç1·d?€ñ€Ýg ?©ç1·d?ïZRÚ þp?‰Óòl)Û?"µ¤±›ì?‰Óòl)Û?ïóaÁ»÷'?Nßz¹Ñµô?Y<|w'»0?Nßz¹Ñµô?ïðþÆL³•?a°Ó|U?^rûe§?a°Ó|U?îÑTÏ÷4æ?´†#'
Áë?¢ê²ÿ°Êš?´†#'
Áë?íã(æ63?¥f0Ñþ?°æ¿¸ÎNh?¥f0Ñþ?ç5¦"?Š©™Á݅'?‹\9u¯"?Š©™Á݅'AGN3FGL J2157.5+3126@U0m_êKcÀ2=²?'ÌÎÀ7ž1œZ>:À:ôŸÅ,Å[?ýºOq­A@¬:ŸŽ%G@¢ø{§@¿Ý9: Íâ¿ã–δ¿ û¿æ_8`ÞUû¿ê¡¯`¼iŽAGNfsrq@Òg ù	lLogParabolaB2 2155+31?ïÛ)±K´V?rdÇ-½.Ê?rk'Z%Õ?rdÇ-½.Ê?ﬖ8¼	?'Nh#òüÌ?"øڏm¡?'Nh#òüÌ?ê/ÞN¡Æ?²¸ùÌ@R.?Ç@†Åxçë?²¸ùÌ@R.?ïó[0A*1?D^vÃM	Ó?YIŸÒáîV?D^vÃM	Ó?îòžÉëW8?¡á'!ãÆ? ÖcZƒ?¡á'!ãÆ?î–>©;«°?·"mÏ+º?¦œo´àö?·"mÏ+º?èTÔLaÇ4?²ŸæQ?ά®Îxã/?²ŸæQ?ïòÉzv­u?T#x…˜ÊØ?Zm
á*µà?T#x…˜ÊØAGN3FGL J2158.0-1501@DOs€*\ËÀH ö½À9+äŠYÀ;"C/Ш¿óòúX¡,@^‰x9M@'Õ`EK¿ãyGë=|¿ãàã»âÕß¿åu(ÐGšb¿Ûª{4åÍAGNfsrq@ŽG¾"åÞPowerLawPKS 2155-152?ïÿ"Ò–v‹?	¤ÈøÎ?SÇÁfç?	¤ÈøÎ?ï×Îʗ­?z[Øïtr?tš›l@'?z[Øïtr?ïÍéV#M?u'ÎÀ^'?yuàT?u'ÎÀ^'?ïÿ÷kÍj>É÷>UF¨>Ñ)L·'>É÷>UF¨?ïþÜäòÞY?&Ԟµ?"1­±¨¡?&Ԟµ?ï?½Q˜±?¤µçËÙ?˜Uß¼…Û?¤µçËÙ?ïP·ù´•?'/¢É²ÕÅ?•ð	ð×Y?'/¢É²ÕÅ?ïÿ¡Cd·B?	+¼|?¯.𳶟?	+¼|AGN3FGL J2158.8-3013@1º¾`"‡ÀJã?ÕØåÀ60Õñ8¼àÀ9Ïù‰Ä:?ðÚº1¦k@µŽM5<ù?ûCÁñQ'm¿Ò
¡ÞPr¿Ý[4Z5窿ٯ ›¾7¿Ú@µwp¤ÙAGNbll@Œ@:>À/0LogParabolaPKS 2155-304?îœv|DZ^?·®ì}pT?¦8˜?)ö?·®ì}pT?ïގ‡±~?'oÉr—?p¸¼%àçB?'oÉr—?ê$Q²
?³i
–³¹•?Çoª¹7ÕÀ?³i
–³¹•?ïÿ&2U?ïù厚0?|œm'_S?ïù厚0?ï¿ìK'{?‹rÁe%ù®?€íB=³.?‹rÁe%ù®?ïV¢–ìú?¢°Y•ñº?•+­A'ü´?¢°Y•ñº?íÁáŒL?ªôŠ—MX?·Kñð…ª?ªôŠ—MX?ïÿ3)"89?ôê·÷v?šÓø"9°?ôê·÷vAGN3FGL J2159.2-2841@4<ú?̞ªÀJ¼ .ßÀ:¨y0nÀ;´ÆžµbM¿áäò
¦f@Øe-VOm?ÿSßûþ"¿ê³A¥*¶&¿Ü1''©Ô¿Ò	nÕ1˜¿åG‰óD—AGNbcu@©Ç\'ÑNPowerLawNVSS J215910-284115?ïÿ/<¬?:Ó²¨à?€\iS?:Ó²¨à?ïÚ§HƒÒ]?"ÿb1‰¡?r¬[­˜±•?"ÿb1‰¡?ïÙeáJ!%?u$ÃÐ(÷?sMDñíˆ?u$ÃÐ(÷?ïþ%-r:@?ËÙwÔÏb?-­+­£r?ËÙwÔÏb?ïþ6âÈÀ+?+BþUo?,'Ö[B_Ì?+BþUo?ïlÝLæ|?ŸÏ–Y1ðI?'~dRó"x?ŸÏ–Y1ðI?ïºæD[éO?áåйG]?FnïŒîM?áåйG]?ïó>ìØcŒ?QðOu>Š?Y'&‹²Â?QðOu>ŠAGN3FGL J2159.8+1025@QFàà¨.À@ú0ߛÜjÀ:þñ´
À;µu	—Xw¿ÓK!ÄÿW@ùô+¶g0@% Jù#¿êS?V›ÜÚ¿éλžônʿȑDá[z$¿ïï{¹ðã>AGNbll@ƒ
:'£PowerLawTXS 2157+102?ïü÷ìz?3'›ð¶¹?8@žKÛ¶\?3'›ð¶¹?ï¨Ö‹<‰ž?œ™‰…M§ì?…Ê]-mü|?œ™‰…M§ì?ïcAý6³,?…U¸¯Ž—k?"—ÀRJb•?…U¸¯Ž—k?ïð*"¢&?Iŵ(ÂXÊ?_ªÙ¶´B?Iŵ(ÂXÊ?ïýTÊ»-F?9iO'µˆ÷?5YªK÷øS?9iO'µˆ÷?î¿:›$?´<xžz¾ˆ?¤VN¼É?´<xžz¾ˆ?ïUnÕu¾?'mÛĚè?•OÒrQ?'mÛĚè?ïŒ>¹V×?…xyìޘ°?ŒúpG[vX?…xyìޘ°AGN3FGL J2200.2+2139@S'tÀ0ÝÀ:6_7üÀ:°àÝûÉÀ;Ý`ÖÚlÉÀ.Ð ¿=B@ŽdŸfã?ÿ£k_I'™¿íx[â»ã¿Ç	$6@-í¿Ø]Ÿe`'¿ÒQh3VTÝAGNbll@¯I$oiPowerLawTXS 2157+213?ïÿ¬d**?INò¼)?Šu'â?INò¼)?ïÏû^
Z?ƒ\)k(¹?xQ
ð À?ƒ\)k(¹?ïÙJ6ô£?rÎm'vô?spZâuê·?rÎm'vô?ïÿþbœ~>¤<PÊ.½}>©Ôú¦ÅP>¤<PÊ.½}?ïþ
eøÐ?)BÝÝzï?//ú®íÝ[?)BÝÝzï?ï ¾ènÏþ?­'£ÉüÁe?›è"õ•œI?­'£ÉüÁe?ﯨ'P—??"F¸!ú8±?"Û®ñÖV?"F¸!ú8±?ïÿÕ
õ]>ùÜ%'Òª>õxïà"Q>ùÜ%'ÒªAGN3FGL J2200.9-2412@;}"V!uÀIÓÝà‡kÀ:H%"ü|À;â½ F?¥½9…'‰Á@e›»2@¡³_¾V'¿éƒëûnÔR¿ëuÄÓ·«0¿¦õ§•
vi¿ã)åz©Ð…AGNbcu@Œ©%®æ1ùPowerLawNVSS J220036-241428?ïÿ»ª™#Ü>úכ7á6?HÏ[œž>úכ7á6?ïÌ?6K˜?í"~ž?yàd­ÌOþ?í"~ž?ïߖ:`ñT?q>G?Wú?p4âƘZ?q>G?Wú?ïù㿾­‹?3˜§¡¹êJ?Hqav"?3˜§¡¹êJ?ïÿÅSlõ³?ÛnÏS+ã>ýV:"ÆÅé?ÛnÏS+ã?ïVz¼ù^ë?¢0Ͻ®Q?•0¨`Ô"¤?¢0Ͻ®Q?ﳗÂ)Ü?'1áÂYٟ?ƒ"…ê?'1áÂYٟ?ïé? sµQ?`—Xã¥8*?fÀß«ç?`—Xã¥8*AGN3FGL J2201.7+5047@Xi"d¯À^ƒ¿èÉÀ8).‰À;5/»¯n?îkÀÀSJ@r'2Ÿºp@¶Óàg^^¿ä$`gÒTÕ¿ç6ÃÝ©­¨¿è®n4]w!¿ï3Š!oAGNfsrq@zÿž£Y5üPowerLawNRAO 676?ïô<Ë7vd?RåÌX%²?W†iÞ
wÖ?RåÌX%²?ﰝ»¬ë?"ë9];s?ƒØ'§X?"ë9];s?ï
*ÕÙD?'ØÎÁLC®?žZ­ì$†?'ØÎÁLC®?ïÿíÞ6Îì>ÔÈG߇¤×>â"øšà>ÔÈG߇¤×?ïêl%JÅÕ?f£?"‡'?e"Ú½y;a?f£?"‡'?î0{™™Í?»KÐ/z8x?¬øFgâJ4?»KÐ/z8x?î•J5i‡?šéÇ'Ë?¦«\«Փ?šéÇ'Ë?ïÿð 37>àéH ^æù>Þ¿Ê]!½è>àéH ^æùAGN3FGL J2202.4-8339@s?÷LÀ?¼±v/À8}¨'j¨ëÀ;³¦‹¤?ú>ÿ'ö×@ºæ´Õ_C@"?(ßÈ'¿áðÆËÅ«¿åÁªRàˆÓ¿è¤ÃðÉðé¿ïW¶ð9üAGNfsrq@‡ª¸Që…LogParabolaPKS 2155-83?ïMâq#Ù¤?—›"!ړ?–C±à¬5z?—›"!ړ?﹚è?•ŒÞÿ^?»™rO!T?•ŒÞÿ^?íÂ¬G?Ÿ·¯˜Ú8
?±ïŸ‰ÃnÇ?Ÿ·¯˜Ú8
?µ}>´?sHkä¡Ë?ŒÒ§Šÿ?sHkä¡Ë?î%C5ßµÞ?¬VhöYP?­«Ì LÔ)?¬VhöYP?îŒíCÌ¼?¹삶z?§1+È»;?¹삶z?í3½<"Žv?¦Ös›þÛ?¶bMÑ?¦Ös›þÛ?îë—ÿ©³?"˜gtÁ8"?¡FŽ>M–×?"˜gtÁ8"AGN3FGL J2202.7+4217@W&@_×,À$á'ÿùJÀ6t _ñØÀ:…nÉw-?õôò°·@0áhv@ã±jƝ¿á€…15_¼¿ä©§…âÏæ¿ãÚÓíõ³Ã¿å±ë`œßAGNBLL@u¾l <K
LogParabolaBL Lacertae?ïýE&6Ý?="^ªkÑ?5ÖÍXm<_?="^ªkÑ?ï´Gá§5 ?"E!kaWF?'î‰|
&?"E!kaWF?ïWÝÎ
$è?•lu:'Ä?•F5Ä]?•lu:'Ä?ïÿÀ^CF>ñ©3}"1>ÿÐƔMØ5>ñ©3}"1?ïöY£Š^=?Z3×5Äý‡?SL¹Kx"à?Z3×5Äý‡?îɏùæ>?¯)°Ì'Ê…?£gbx¥?¯)°Ì'Ê…?ï$wxKÛ?—<EbÕ?›qo>¶¦?—<EbÕ?ïÿÔ[·`Õ>÷ç#)H€,>õÒ
Í~Ï>÷ç#)H€,AGN3FGL J2203.4+1725@Rëà
ò1À=£GàiaÃÀ7»Šˆ"ž`À;Šrµ)B?ñååóö@ڜ#·•-@QâZþ~K¿ßð0$ò¿ãðk"LD@¿æ!ÓÉã…ÿãSù¼;|zAGNfsrq@|wýAt>–LogParabolaPKS 2201+171?ïÿšý}?vCä[è?,°ÈÌ=?vCä[è?︠âRû?"¾¿ÛÝè?×Çl…£9?"¾¿ÛÝè?ï íYpoæ?ƒönñ¢1ª?‡Ä©£ä‹?ƒönñ¢1ª?ïûrú?îû?+0¦gàÀ"?B4©ôKØ?+0¦gàÀ"?ïþÛI´¡T?&lþ•Š8‹?"Kcewcâ?&lþ•Š8‹?îöµBäÎn?³æ¨½ÖÊ? "«Ñ³%?³æ¨½ÖÊ?ïéò;`?–µ\È?œbÁ¶Ü/?–µ\È?ïöà3S`ó?Ið®÷™?R?™7Ú³?Ið®÷™AGN3FGL J2203.7+3143@U¸¿ÏŽHÀ2ރàÊ°"À9 Qðœ5À;Pf͔ÀŸPõ-¿@'=Ì¿5à@†‡_ZX'¿çšøO:c¿éWÝ÷cñŽ¿ïÿÛ¾"_T?ÚW·€¤AGNfsrq@t0îËûµPowerLaw4C +31.63?ïÿÔx+¥?#÷´˜ßxh?x¾v0Z?#÷´˜ßxh?ïÉÈ:¨?ŒüÿÏÁd]?{wËN¦¹?ŒüÿÏÁd]?ï§:Mr"_?†çúEnÄ?†1l±˜!?†çúEnÄ?ïÿÿõC8>UQ¼™Hæ´>UmJK¤>UQ¼™Hæ´?ïüŸ]?@š»&X8Ü?9ëи«?@š»&X8Ü?ïI­•qc?±(G™]
ì?ŸVÊKš›?±(G™]
ì?ïc䂏֑?ŽùaSvã?"ƒoª•'ã?ŽùaSvã?ïÿý儺Ë>ºXPý<Õ>°ÓOÇ3A>ºXPý<ÕAGN3FGL J2204.4+0439@P.lŸÐë?ÀCSçÖyõÀ9îévQÀ;Ãr°÷"0¿Âîªzüö@^Óª¬±@þ=ß^ŸÉ?Ùlé™BS¿ÚB»ú "R¿ëM豍^Ö?²uµ"(üAGNbll@›hwškQPowerLaw4C +04.77?ïûÖ<Y™ò?Pp¸Ý~6A?@§ãC7?Pp¸Ý~6A?ïÃè]T¢w?<^[ÿ$ü?~ÑuK,3?<^[ÿ$ü?ïŒ*_ú?˜JFîX?Ÿ.zµÕnÅ?˜JFîX?ïþ¯&.ùú?4~Qj®p?%
›àéL>?4~Qj®p?ïè
žÝ?nQQø^¹?gõ:…3y?nQQø^¹?î¢V%ÈÞÎ?ºB9BcIH?¥Ú w%?ºB9BcIH?í#nCrV?®ó´–k?¶äçª`Ì?®ó´–k?ïíE¢ÃÜ0?dg+£hðš?bº]{\Ÿð?dg+£hðšAGN3FGL J2206.9-0031@Mú¼ßï¿@ÀE6ö`D
vÀ9¢T™µHLÀ;ªf̽³T?ÐXá"-nÎ@Ûhêz1Ê@üâo\¿×âK€K¿âæ‹Ôx×q¿ãï/Z¶"â¿è~ %ò$mAGNbll@'^³üPHPowerLawPMN J2206-0031?ïöïåÍò?|åb¾è¾?R 48 ïÃ?|åb¾è¾?ﳏoÛ@i?™b¯~†Žg?ƒ$¨?™b¯~†Žg?ïµIɀD¼?'óä¶úI?'­'ˆVô?'óä¶úI?ïÔ<ÅO¢L?Wç<¾?uái\åß?Wç<¾?ïùBœ1Ï[?PIà>ÍO?JõŽXu¯?PIà>ÍO?î~¼Ì­ç?º€êœÒšR?¨35.'?º€êœÒšR?îӕÅ?œžÉš˜f!?¢Æ¡v¨?œžÉš˜f!?î¹óA^LÅ?ŒŠo'Ü|r?¤`Ëé?L±?ŒŠo'Ü|rAGN3FGL J2207.8-5345@u>…ߨq¤ÀHøm¾iÀ9ôÛö5À;̪â—9m¿÷?´öÂ?@\Ý%µ@ªå_ë¢ü¿ç~"ƒ
¿åCîÛ{¢t¿éjÄzÔç`úû©ëAGNfsrq@}Ê˜ñÔPowerLawPKS 2204-54?ïÿ,¡ÚÁé?"i^"‰RZ?kÀ{	-R?"i^"‰RZ?ïÌ@íë—?Û3®2vØ?y߉P=à?Û3®2vØ?ﵕ%?±W8fœï?'š½,(Û?±W8fœï?ïÿúFW¨3>À³ pñ>Ææô÷À¥v>À³ pñ?ïÿ˜Sڄ?š=Çdà?Líqš|?š=Çdà?ïDƶˆ<Ð?¬é Iåeñ?—g)5םù?¬é Iåeñ?ïlؘ²éÍ?N'ȳ?'dìîÊ0b?N'ȳ?ïÿ³×ˆg˜?t!ô>?

ÚSw€?t!ô>AGN3FGL J2212.0+2355@TŽH¿÷Ò4À:©?ÿÊPÀ9}K…9À;†ûß	?ÕKêßâ@,þ¯çÝ@²Ô (>Ž¿àÓý鮿☐MH:à¿ã«Àsß1¿ãr`†Â@FAGNfsrq@"Å̈́M;PowerLawPKS 2209+236?ïû¶Ó¢e+?I‡óŽüϼ?A$±'ÍÜv?I‡óŽüϼ?ïµŶ­¢?18hCŽµ?'©ŒêSWU?18hCŽµ?ïÂQ´¹Â?Ë¦¡/á'?~ýWCß®÷?Ë¦¡/á'?ï©àî0¹u?hÜÊJ±?…‡Ä~ v«?hÜÊJ±?ïìÊ J"c?gJíã«?c5ßÚùdË?gJíã«?îfœT½?´ø?.x•;?©Ÿß¢Ë-?´ø?.x•;?îõه+"?—Õÿ®ÿåÜ? ¢g‹ŽðÇ?—Õÿ®ÿåÜ?íÂm+C? ìéØ[?·Y엃Äå? ìéØ[AGN3FGL J2212.3-7039@sôî²ÑÀD‡"€,á
À:${À;´»¶úÓp?ìû–dìúÑ@9`؇ëò@}\¬~¿ç£ÿ¦5UÅ¿è^VÚN·ë¿ìJ¦b2'½¿ÙaÿrAGNbcu@‹T€uPowerLawPMN J2211-7039?ïçîÿÛ©?pcnàļ?hb¹N9?pcnàļ?î
NŸÂŸð?¹H±RäM?¯[ú?¹H±RäM?îìN@ïx7?"WÐ:g?¡;ïP®?"WÐ:g?ìîckÆ]Ù? ô½9ƒo¼?¸Œä£òÒµ? ô½9ƒo¼?ï¶Û.I%?é…ü?'I>ç_2à?é…ü?ÝM{šs&?Óà"=©a?áYB2÷Æm?Óà"=©a?ìë‰Amï®?¤kœ©k	>?¸£µóF¨?¤kœ©k	>?Øi‰ëj‹~?Å*6ŸÏ=À?ãË;
JºA?Å*6ŸÏ=ÀMIXED3FGL J2212.6+2801@UK2-LiÀ6û.Àë­À9ðÑ@±¡À;Qøñ?ÞwՋڋŸ@
z£?	Ö?ü¥ôÞä§_?îñÇ53=š¿Û⦖ŠÏ¿Ïáì"b½¿Òې
m•žAGNbcu@°QS¢œwšPowerLawMG3 J221240+2759?ïýÕz4=c?0ãÛðՕ?1T,ʏ•Ç?0ãÛðՕ?林.<Ë°?˜ätX&?†ôt<°
?˜ätX&?ïØ7Ò²Èr?jYÍ…»¬?säšíç?jYÍ…»¬?ïÓn/°?Y÷Ä0<Ñ÷?vH¹MHV?Y÷Ä0<Ñ÷?ïóm½?¼?\ÐΤgLÆ?Y$Äótb?\ÐΤgLÆ?î€/¦>v;?¶x
ŸC¼?§ýÐjN?¶x
ŸC¼?ï¤1Û?…¾Ëç¦k/?†ó¾‹èíD?…¾Ëç¦k/?ï\›‡A?'_±§""?"Ï̏é?'_±§""AGN3FGL J2213.1-2532@:UC_Ñ ïÀKQìàh‹À9™TpšÀ;Ñ&çËUÔ?¼ŸáA+¢@íÓW«c@`e@ ¬s¿ãŠn'!¿åÌ3[t¿æ¬K¹xz¿ïÿõ•æ(5AGNfsrq@z¬Ùè>PowerLawPKS 2210-25?ïùnù²Þå?p$*¯f—‡?JD{üK¨?p$*¯f—‡?ïÐT®Øðò?†BŽfõ?wÕ¨¯f¡?†BŽfõ?îζIŽ?›ì4¡;\I?£t—#$?›ì4¡;\I?ï¾&fú"?e 9Zc~£?€vf6fÊ?e 9Zc~£?ïðQ`½&‰?o-½—>L?_]>Ç«m´?o-½—>L?îÿT€Ø$?§-P!Ø? 
·óY¥ú?§-P!Ø?sW;?íW™µl`?§Öo»^AR?íW™µl`?í¤ø :?ŸþC¾ûç?²Ø?¾ÿ&3?ŸþC¾ûçAGN3FGL J2213.6-4755@uÀAà?pXÀJ"õƒ¥À:Ú'ˆ-aÀ;òABÀnð?dz¼G:ôj@ÇÉÅÜB·?þ;þÝÁ¿èeêG(ó¿c>"0hê¿äxiRÿ×;¿Å1݌|iAGNbcu@ªˆ#9ÀëîPowerLawSUMSS J221330-475426?ïýFŽs‰?2³÷«Øx?5ˊ˘"1?2³÷«Øx?ï˳þR^z?FÀƒLë?z&ËÒñ?FÀƒLë?ï«|_÷âO?»á ¡ÿ!?… èÅÜ?»á ¡ÿ!?ïêÔ_=RF?Q‹²Û!ã?e+ ÁMâ?Q‹²Û!ã?ïø»*ìp_?N&:u	ñM?MSI¨ó5?N&:u	ñM?îå+ÔÖAÒ?²Ú¨Í¿!?¡­Bµ/—à?²Ú¨Í¿!?ïX‰/­Üa?'i#¼ì?"îÚe;ù?'i#¼ì?îåôÃDe?–Aÿ
m¥?¡ ³Ê_n¬?–Aÿ
m¥AGN3FGL J2214.6+3000@U¶¦ßÓ9ÎÀ5ª¢_:øúÀ8"kp'b"À;k/¬•õ @1Tc¯}@¦ÃMÈ
?ûÑE'ñ6¿œ³š~V·¿Û˜Û¥úó¿äºˆ‰&¿îwe_*\öPSRPSR@>°‰ 'RPLExpCutoffPSR J2214+3000?J?‡Aÿ?K¸²º·ß"?ïùpcE—?K¸²º·ß"?°'žEÍU
?×ÎEüA7?ííÌ7aÒ>?×ÎEüA7?Ÿ.ŸÎ݋E?"½œã?ï‹{U6?"½œã?sŽÙm?]Q¼éÚï?ïØãÍß
V?]Q¼éÚï?O'"ÒúP?E¤µå[?ïø8[™·T?E¤µå[?šPêÙF:ž?³ï('`"?ï-x©_	{?³ï('`"?ˆ3Ft¾y?'§¨Þ?ïŸ2æY¶?'§¨Þ?I\b?AÐ*Å9|?ïùœ)ì?AÐ*Å9|PSR3FGL J2215.6+5134@X÷ÏÀ1³×À¹vÁçAÀ9žý†¨üÀ;WÊÆb?þ¥y+û¶@)"×ëŽÚ?üÕJœ?Ưåi'I¿Ûön+¸ý¿ä\z&.4h¿îÜ)µþLPSRPSR@"&̘_÷PLExpCutoffPSR J2215+5135?HªK̛§(?DÒd 2`M?ïùÕlê .?DÒd 2`M?®9V·'?ÂÍñC·?î¬jy?ÂÍñC·?®?¯÷·®™?Ÿ@íªÅ?î'C†?Ÿ@íªÅ?»‡gŸÃ̕?—	)µ¶#Ì?ì†m?—	)µ¶#Ì?Q{2÷Í?_úP'h?ï÷BuàÌ?_úP'h?U–ì£e?©awÃtÎ"?ï}SO)Ö5?©awÃtÎ"?@†(D?…Í-éÉçþ?ï}ûƒ÷úV?…Í-éÉçþ?'Ô½ºª?xýÕÉl»U?ïi_ö­Ï?xýÕÉl»UPSR3FGL J2217.0+2421@Tâ5`4>À:u§€)ÚÀ9;ٕ2+ÌÀ;‹õ'¾´?ä'ú¾z@'/ó7Ŕ@¸Š`¿Z¿áœ坠‡¿äÔ]eòßA¿ãªª=€¿¿àãšæîAGNbll@"e)ûçl‹PowerLawB2 2214+24B?ï/["­p³?¼`˜
?²?šq1!‰?¼`˜
?²?îœLæ§X8?­Å>ýêó?¦;1"®•ƒ?­Å>ýêó?ïVcµÈ£?˜£"3?•3‰^&ë–?˜£"3?ìÂê€p^?›[¡Ðð~ö?¹è«ÿ¼}
?›[¡Ðð~ö?ïÍÞT߀Y?"ÊÖäŽñ†?yՙ.Ϟ?"ÊÖäŽñ†?⪋‡EÅ?ÑEœµ¿?Úªèññtw?ÑEœµ¿?í®€ØœR ?¤¥2Á'ºö?²‹ù;‹^}?¤¥2Á'ºö?ÙµmÂr£-?¼<'gMìó?ã%IÆ®i?¼<'gMìóMIXED3FGL J2219.2+1806@SÜÝ?á—_À? íàBËWÀ9ö-Å5(×À;Ålґ2¿åŸLv{1z@Pš¢-@	qŸŒ¨¿áöͅô ¿è^ß®ü­:¿æˆ#Ó¢\"¿å¶"ÞAGNfsrq@‡¯(Xy=ÙPowerLawMG1 J221916+1806?ïÂÔ>æÆ?µpEd…ˆ?~ž5ú©¥?µpEd…ˆ?ïÒîO‡t?".7lœ,?vˆØ-_}ú?".7lœ,?ïá'uwÉ?tØ0¿KÁ?n}Š"§¾Ñ?tØ0¿KÁ?ïþßàêÕ?fD#¸-=?"óȈ{?fD#¸-=?ïÿ˜m÷G?ó,y?	äÊÛI^?ó,y?ï
Bwš?²¾Ï󘟑?ÞW«æâÈ?²¾Ï󘟑?ï³V1÷?…âêÿ~Î?ƒ?*s'>ð?…âêÿ~Î?ïòÛ9:ù?Qügû­ ?ZäIÕíË?Qügû­ AGN3FGL J2220.3+2812@U°p@üÀ7ۚ?±Æ·À:†Tò ›ìÀ;Ëö³P$¿ê!È!õѱ@
SÙñÎd?ýU'Á(¿éð…ӿ݆³Äí°¿ÕjäJúm¿Ë²¹¹­AGNbcu@³ˆ -àPowerLawRX J2220.4+2814?ïÿ·-Ü»?aZVRû•?)ûwùt?aZVRû•?ïј•~q?ƒðÞ2Ówn?w3ù©'´?ƒðÞ2Ówn?ïæLév?YÜ-%œ®Œ?i³ïYâC?YÜ-%œ®Œ?ïÿœ,h`3>úóñ©9©Z?ôíû0>úóñ©9©Z?ïþunlY?""î¶õc@?(©c
ìu?""î¶õc@?îð°ŒzLL?±úåpeK? ô÷6£m<?±úåpeK?ïÐ[ƒŠ?w²[KDé?wÒ9o³*?w²[KDé?ïû©¡?>ýªÐ¬gÉ?AY|)Öà]?>ýªÐ¬gÉAGN3FGL J2221.6-5225@uE¸Ÿƒ¾fÀJ2ûÿÀ? À9`^SrmÜÀ;Ó~—µ"¿ü˜V¶E ñ@+óSIS0?þÒ^ß´[¿à+hjìÅ¿àŸÜo4É¿¿Ú«`êG¿ÜšÖœžAGNbll@¡ÉíúCþ]PowerLawPMN J2221-5224?ïú(}Ö"??K*ld?G^g±y?K*ld?ïËÓlgöù?É?›îªå?zIé''R?É?›îªå?ïÅì¯ô
?ußòe+£?}	þ3ºÔ?ußòe+£?ïÿì2Ýf½>áéãìaò=>ãÍ6Ë¡p>áéãìaò=?ï÷¶½ÁÂ?LŒ»'uO€?P'"i>,•?LŒ»'uO€?ï.í𢮰?±eæöBÎ?š"Aëª*?±eæöBÎ?ï~cƒï˜?‹¡•\Lâ?3ƒÓû
?‹¡•\Lâ?ïþ_¨ âR?,
‹(u?*t˜›ºé?,
‹(uAGN3FGL J2222.3-3500@#Lßàû®ÀL¨ñß«Ì¢À:ƒ¸:lãÀ<-*ÛuÝ¿ê‡Z'÷@Þ¬FD‡ï@ùã_`bÁ¿ãU¬žcË¿ßÕÖқT¿èÜÆè1W;¿ÖDf'§ûAGNfsrq@ŒÚÚQÎPowerLawPKS 2220-351?ïÿcÚ½H?£^ß<áK?v^æ ?£^ß<áK?ïßÖúD¡'?€É¿±Š?p'þ«vÑ?€É¿±Š?ïï?F?ˆôeÜÂ}?Œ"05XМ?ˆôeÜÂ}?ïÿóOîTÝ>Ë™<(+2>Ù`R¶1X>Ë™<(+2?ïþ9h£ÏË?3êϒ9Þ½?,ivcŠ«´?3êϒ9Þ½?ˆÄpn?žƒÐ{ûE~?Ž'Ýĕ‹?žƒÐ{ûE~?îÏmä4'?›V½7>ÁÃ?£	!º*à?›V½7>ÁÃ?ïÿ‹°Ã6?	‡Ö#ÇL?
ò
vÒ?	‡Ö#ÇLAGN3FGL J2224.6-1122@I$­€k`ÀJì@/šøÀ9öÌP¦
ÁÀ;¾ðù²¿ÿ9H*¼@
±Q؏Ε@'ªo÷µ¿æ‰¡Ñv¿è³ifƒw¿Ò0ыšÊ¾¿ïùÓKþ'AGNbll@ŠÐéÂ;ySPowerLawPKS 2221-116?ïòc?bècãˈ?[8#	}ØÍ?bècãˈ?ïÒ-ôãZ?†®kUü?véü?†®kUü?îÿÍÌbTð?	8\E? #7Fü?	8\E?ïÿÖ:šì¼>øyyÔÖR>ô⺺Ÿ
‡>øyyÔÖR?ïë·[ÿã®?qrq°öR?dH¤›±à?qrq°öR?ï=a>à?¦Ø›¨5À?˜SÏք–?¦Ø›¨5À?îËËQÈ?—h€®!w/?£CNoŠã…?—h€®!w/?ïý‡eS[?8tH–…×Ø?7[Å3ôp?8tH–…×ØAGN3FGL J2225.8+6045@Z"O~ÃT~@wàmòÀ9܋Ëz½6À:ò
kùM^¿òÎ?`"Â@ŸÓŸÏ¾š?ÿ&´Nߌ?éÅŠ†`¿í 4é옿ҸŠ©³¿Ãê­ÈГ×OTHERspp@Ãé:=p£×PowerLaw?ïýŸE³œ?=ê
àÜìj?3Ñߌ‡?=ê
àÜìj?ï¾ôìóÖ?'$¿óS?€BIJŒX¸?'$¿óS?ï…ü–"¨?Œ·77šc(?Ž€Ú^oqß?Œ·77šc(?ïÿèù(Jw>ßO\́^°>çµ`z®¨>ßO\́^°?ïøŠUX÷é?\YÕÃS–?MÖª‡É?\YÕÃS–?îÁL#w±ñ?³vM¤£ä?£ë=ÆÍõ?³vM¤£ä?ï¥v>4?šÍ$T€Ý?«Q3¯~?šÍ$T€Ý?ïÿ9N³ÊÑ?Ëðâ°?Ö'eJO"?Ëðâ°AGN3FGL J2225.8-0454@M……rÀHj> N¿À8l'šÿÀ;g%ª´t?ñ2KÇ~¯3@F3´7€@Þl ¾4¿à>µÐ[øy¿æOEz³zk¿å€EØ|Xk¿êia1ëæAGNfsrq@ƒãAâXOLPowerLaw3C 446?í¦¤Ô'›?ÌÞÞÛçG?²ÊÙ\Ç?ÌÞÞÛçG?ï
ˋ{–?¢Å!,¬x?ž½f‰i#D?¢Å!,¬x?ïVEòŸè?Œ÷_fz¯à?•?×:ÌË?Œ÷_fz¯à?íÓqŽ;?"r	ð?·dv½š¬?"r	ð?ïé+V‰¾I?|ciš®Y?fÔ©£œŽ¬?|ciš®Y?êùÇ˨'?ÅÜp%Nf?ÄÈàÑ]ø?ÅÜp%Nf?íÑáý"Œ?¢ß£*qUž?±pð¨î?¢ß£*qUž?ãû©'Å2?µÉjșã÷?جÛÚuœ?µÉjșã÷AGN3FGL J2227.8+0040@Pw[À6ãÀFמ_Ñ÷¯À9'|üªàêÀ;"},{‰
?ñ±«®o@6Óü–ê@'?ØÝý?äÒ»Þ+ޚ¿å©`ã<¿â¤ØXŠõV¿ëÎQ":èAGNbll@"‹ñ©ûçmPowerLawPMN J2227+0037?é	hAZ?ÇDïÉ&$,?ËÚ^ûãæš?ÇDïÉ&$,?âÜA˅?Ή/áf"?ÚGï|hõý?Ή/áf"?èXÚa?±ô¥`¥›Ö?Οëô–{"?±ô¥`¥›Ö?äìxŶ?§öî<Ú÷?Ö'ÉÜt"?§öî<Ú÷?Úk3³>cñ?ÏzÑãšw?âÊf&`Î?ÏzÑãšw?Ñà:ÛÑ«?Ëê!.×a"?çâ'*z?Ëê!.×a"?×{
Ûhyš?»aܟÂl?äByKÃ3?»aܟÂl?Ì|BL;þð?¨y|äDG?èàïlñD?¨y|äDGMIXED3FGL J2229.0+6114@Z© b
·@¡àE$¢À6,6*^x[À:tĪ¿[Ë@ž<ÓG:@'3DÐêi@&k×j¿Ø¼˜!I{Ê¿âêÚ»:¿åIÀÐó¬¿ì²Mx6{PSRPSR@"|Em\ú­PLExpCutoffPSR J2229+6114?Q—¿5' ?XÝ;Nœ…†?ï÷4 \ے?XÝ;Nœ…†?¢
¡#飤?½º
¨O"é?îßUíê¡?½º
¨O"é?¬¿œ­ï?¡}óƗƴ?î>Dñ²?¡}óƗƴ?/aó_L?%?#	­îWs?ïþ	àÿ^Å?#	­îWs?Gã"Làµ?CÄ0iU;?ïú%'?CÄ0iU;?…6ÐK²[?¢¸Ç'ò|?ï«$¾Ñ6"?¢¸Ç'ò|?‹D %\?ˆÇlÌÃ"æ?ï'ïîçn?ˆÇlÌÃ"æ?~ܓ™­³?qç±ÛÞ®?ïÿ¦zÒÉ?qç±ÛÞ®PSR3FGL J2229.7-0833@KíàBËWÀIÛÒÀ+ԚÀ7¤ä+Ž#À;Hª9$
ü?ùÐÁÙ©ª@‹ÆùÏq@©x3îD¿ä'ë‹îz
¿çggWÒú¹¿é7dQ캿íàP8bÙ$AGNFSRQ@q¨ÿÁßeLogParabolaPKS 2227-08?ïßx2c!?l|Іg?pCæÆàZ?l|Іg?ヲïm‹Ÿ?'X7}†©?€–D-ä
G?'X7}†©?îH¢¹'ÿM?žF©ÏË'?«uÔo7Ù&?žF©ÏË'?﾿¦H©'?fj@¾-.?€PrMw?fj@¾-.?ïγñyø?wl
;"?x¦pý¤3?wl
;"?ïJ°ÛÞ?­6™²'¶Ò?Ÿ¶©íCJ?­6™²'¶Ò?îӋ96¿?š—¤­çô?¢ÇGíH{?š—¤­çô?e?'¢.Zß´+?8?L÷'?'¢.Zß´+AGN3FGL J2230.5-7817@st­••ÀB8H˒:À9Eg™TÀ;¤`·Ð¼À«]¥wžG@ؗýZ¬@P_"äN¿ç óäq¿å`Hü.u¿ãL
2ïý¿ë[×ãðï†AGNbcu@ƒG‹C•PowerLawPKS 2225-785?ïýßûcõ.?.5ŒH?1&Rß ?.5ŒH?ïÓCúÎ	?Šv-órã?vqÝé+ßv?Šv-órã?ïµÌkº†?~0];׈ô?'ŒåÈrž?~0];׈ô?ïÿÿýPÎ$>M˒ãòT>5CHïp
¬>M˒ãòT?ïýëî{X?4ðµ®rà?0 Š(èß?4ðµ®rà?ïB9ÓÚf?­	ŠfwŽ?—¸ÝE"³G?­	ŠfwŽ?ï"D"C̳?Žü¤Ok±?Žî÷uì?Žü¤Ok±?ïÿÿPúæ³>§~ÊÕÎp>•â¨üG±>§~ÊÕÎpAGN3FGL J2230.6-4419@v³¿µÀLƒT_Ó¥.À:P/žS<¾À<V	!ò¿ã™õ&­ƒ@
ŽYõiÏ@"NàbÖº¿äÌRخǿèq‡DÓ¿Û9'Åö"¿í›oËÑ
…AGNfsrq@ƒUÂã?PowerLawPKS 2227-445?ïû%¯(?Fþ¡+˜5?C"jú'†?Fþ¡+˜5?ïÔá¦èP?‡!C¸	Èá?uñIh›?‡!C¸	Èá?îϐ˜áZE?•·c·"b?£öoV¦µ?•·c·"b?ïùEÈ%?9n8$K?KÒéŽ>U?9n8$K?ïýp3¢Ly??:茰wä?4~bëiC8??:茰wä?ï ý
¢?±¸X+e3‹?›à_öµ?±¸X+e3‹?îÁÊHÊ/u?™
"àÙé?£ã[r!µ?™
"àÙé?ï¨ÆHVäq?zΚ<~ü?…Îmô•·¹?zΚ<~üAGN3FGL J2232.5+1143@SZÀ5¯åÀCJ—à[õÊÀ7X‹÷§qÀ;#¾Šêª-?ü«zŒãþ˜@"HM÷"±@·'TU흿ãv-¨Ò*¿ç·@+T¿é¥*LbaÓ¿è‹隸ÓAGNFSRQ@sEfä:§œLogParabolaCTA 102?ïüæfë‹C?>êTwD'Ô?8ÌÈ"x9?>êTwD'Ô?ï¾½¿àøu?',età
?€Pˆ4œ?',età
?ï8[RÙc+?'¦±JÿA?˜ô•Ÿ¬0µ?'¦±JÿA?ïûǨoŽ?0fà9\1J?@á\ñæF)?0fà9\1J?ïöX=r–?S_âãjk)?SO…\ÌbÝ?S_âãjk)?î´0×I?¼£^`ÕÐ?¤¼ÿï÷º°?¼£^`ÕÐ?ï•ŠžÝ"?˜1Ø•/"?œMN­Ü'?˜1Ø•/"?ïûû¿å™Þ?;œÕýn?@ýU?;œÕýnAGN3FGL J2232.9-2021@Bºø_øŽÀLÙÌÿøsDÀ:A±Y©¿'À;ϳt62ÂÀG-BÖ¿@×3#žì@¥ùÿŠå!?Ç%£ø%M¿èFz™Šf\¿Ò_½m'Üj¿å+ñSAGNbcu@ž»d¨ÁTÊPowerLaw1RXS J223249.5-202232?ïü/GãÖ?lÝOþ"`Ï?>…Á4Öv]?lÝOþ"`Ï?ïàÅD9¸*?{(tA1)ï?o:»ÖÅõô?{(tA1)ï?ï™Iun™?‹çL_<?‰­¢Ÿƒ'»?‹çL_<?ïÿøøò!>Ænäïï‡>ÌËóää‡>Ænäïï‡?ïüÊ[áÛ°?M«3Â#*?9­!ôž•ñ?M«3Â#*?ïeC`IcC? rZÕ'~
?"W"ñ¬-°? rZÕ'~
?ïL=æj'«?'Wª†²ÔW?–xC0÷ܪ?'Wª†²ÔW?ïÿmýo¾?MÿܚŸP?@Q\¸õ?MÿܚŸPAGN3FGL J2233.5-1235@I&û?¦ÞüÀKR·?œÎÀ:N(´T0À;µŠª¡¿ü@Hð^Í@z}[‹a@û!_Ìr¿æk½à˜(¿à>Ó	Y)¿âR~WsÚB¿ãº#r AGNbcu@"ïhۋ¬qPowerLawPKS 2231-127?ïÿ	_ûZ? -õ3:?Ô)\Ž? -õ3:?ï×=tø?~…ðûÆè?t}ñ\v?~…ðûÆè?ïÄ,͓q6?vãoãªT?}é™O´€ ?vãoãªT?ïÿî¢,»>Ýì©¡†Ê>á]ëAùi>Ýì©¡†Ê?ïû'Ll¸?DqĂb}ì?A÷æý"Žt?DqĂb}ì?ïEڈÞF®?¤#¶R1Ý?—D®é^":?¤#¶R1Ý?îí׸§ë†?˜ãQ´Ø®:?¡""sÉy§?˜ãQ´Ø®:?ïþ¬ÄÕè?%i,Å$Ô?%3²ÄÁÆ?%i,Å$ÔAGN3FGL J2234.1-2655@9N¡¿ØȄÀMÂ'?ßéàÀ:êÛ«ŒáÀ;é"C÷¦•¿¸cðHà–@,¶Á™®@ÿ²}@¿è ‰	Ôj%¿à'<\kš¿äžª|.¾s¿×À<­Ò®AGNbcu@˜·ÁTɅðPowerLawPMN J2234-2656?ïþÀËjT»? Þ:«,¼¥?#óGÙà? Þ:«,¼¥?ïØ»Á?XŽ?…c×[j5³?s¢P……?…c×[j5³?ïË!ëÂ~?wÇN¤xþÃ?zo7ž¼i?wÇN¤xþÃ?ïû9¾tN?0-ÁeäˆÏ?Cb,)?0-ÁeäˆÏ?ïü_²~S?EØ¥4ò7??ý|…ï?EØ¥4ò7?ï†îMô?šs{G«¤?ŽzeÛË?šs{G«¤?ïsZô ?àqaçÞ?£)?ˆcä?àqaçÞ?ïÐÁäfqy?m•4šekE?wŸ
ÇGã~?m•4šekEAGN3FGL J2234.8+0945@S "AÀD8G@0q¸À9"h¸P>À;ž
§ù®­?ú$ÉñP9Ô@ü¼(º´F?û¶\/Ö²T¿¿aÊ®Q¿Øý˜MY¿ç]RÑÅ@¿íò'³e6PSRPSR@"ôSŽóMPLExpCutoffPSR J2234+0944?šMÿ}©B?¡¯•LÜ?ï-÷9?¡¯•LÜ?ÊG®Új?Ê"|Rr#ð?éznI|å?Ê"|Rr#ð?Î"+Ä)C?²#ˆùÁÖ?èwuõ¼/?²#ˆùÁÖ?Ô.Ð\>`?§ƒq›ñ1?åè—ÑöàÐ?§ƒq›ñ1?wXξ¸?'úÆkÅ?ïÑNd!?'úÆkÅ?¶t'qXÉ?Ž«)C?í1m±ðc¼?Ž«)C?¥½Ïø´è?²ô=çݘ?î¤#=Æ?²ô=çݘ?«¦ïš6Šq?'<Ìh[?îE'x9?'<Ìh[PSR3FGL J2235.3-4835@u‡É¥ÒÀL1@ìFÀ9?ÿxÃÑÀ;Ï3ÿáÍ?å©1°¸UX@·VƒÁ@æÄÀ8ê­¿áø4Tª°¿æp)Ý'¿ç­;)¡¹ú¿ïÿ§U¢|uAGNfsrq@'Haaä÷fPowerLawPKS 2232-488?ïþkbF«?*1vH"?)IÙò
§?*1vH"?ï´¡ƒ"³?"=ñ'WÁZ?'ן!b(?"=ñ'WÁZ?ïW[Á5¯?…Táû?•""i®0?…Táû?ï1D	‰?~þìÍ?™×~×vsû?~þìÍ?ïÿ¶"YÇ?&¥Å~?É*Ë™Ë?&¥Å~?íõù¯
Q?¸»vMº?°P2†/Ç}?¸»vMº?îû¼˜?•Ý:§GŒn? Nä>®f…?•Ý:§GŒn?ê<ChƤ%?°ø˜×¢ŸÅ?Çò\åol?°ø˜×¢ŸÅAGN3FGL J2235.6-2319@@.Vßà¥ÈÀM"
Ÿ–2ÝÀ9¥aÈqô9À;ÒaCöÈ?êô³JF†@ÐÎäÿô@‰¯ÀL‹Ê¿æÁd»ã½Ì¿ìm<<'x|¿ã@`óaK¿ï¯òuÝ
AGNbcu@u·O QC¿PowerLawPMN J2236-2309?ïüö=^…F?:[³d'*?8NÍüˆ?:[³d'*?ï£+õa?˜dùÈ7?‡5v×¹?˜dùÈ7?ï`úlJ߀?‰†æŒÝ
Â?"à²}ƒGú?‰†æŒÝ
Â?îôÚùÇgï?+©,
†? ²P_=þ?+©,
†?ïþ@LBÆ?+ýgôÈ82?+û=¬h"9?+ýgôÈ82?îä"óP?µ¿-yß?¯¶³aÀ?µ¿-yß?ï$Km‰?–óۗ[tò?›}•¾yÀ?–óۗ[tò?ë ÓÕT°±?¬­BA8È?Ã|°ª­=:?¬­BA8ÈAGN3FGL J2236.0-3629@	tŸå
5ÀMöWŸúëÀ9lÙÑ.[À;Âßp=½?ܸA_r@á!c|ý@›ú¿Ï8b¿Û™`GØ«¿äø—'=J}¿ãêĊð¿¿ã4dœÈßAGNbll@X!–R½<PowerLawNVSS J223554-362901?ïÿ —˜@1?èLãmâá?ÚÓ1ÜT?èLãmâá?ïÏA.Ÿ£?"3šhíï?x_iæI?"3šhíï?ïÓù(UÈ?~ìõ䁠?vl±ÓÜ?~ìõ䁠?ïäüU?f?P®­eFi?k뵿Y?P®­eFi?ïÿª‹Õ?ՙ5{?zVa/r-?ՙ5{?ï\Êbܐ‡?¢Óž›&0?"f³›Öé9?¢Óž›&0?度mË,?‡0"T
Þ?…ߤ'æ*À?‡0"T
Þ?ïY6÷|½…?'œÀ?H³Ú?"Ù!G‡c?'œÀ?H³ÚAGN3FGL J2236.0-1706@EÌ)ÿ­Ê©ÀLšŒ 4RîÀ:N×úþ8€À;ÓÂ¥+ž¿ôsÎq»@@å""@
3 "ÉK¿á™»&ÿj¦¿ÕTR|¿äÖǪ¿à"²k;|AGNfsrq@ ¸üPHPowerLawPKS 2233-173?ïþœsú´Î?"#Y5¬?&8Äá¸ó?"#Y5¬?ïÛUŠ1Wø?'¬BN";?rU;@Û?'¬BN";?ïÃ$ƒ~5v?v$ÕH«?~m¾:µøé?v$ÕH«?ïÿÉ~¹™i>ñ•4óóŽM>û@'ÜV»>ñ•4óóŽM?ïûñ71¼Þ?AÉ9ýmoå?@;$!ÀÉ?AÉ9ýmoå?ïD¯*H?¤2`3ù*?—j&›E?¤2`3ù*?ïsé$'|ƒ?Œ3èb÷¾?''ÛxGuœ?Œ3èb÷¾?ïü;(0[ú?<c"$"8?>&½ºƒ!y?<c"$"8AGN3FGL J2236.2-5049@uNß°Õ ÀK"î²ÑÀ:,M…>À;ã"q;¬~?֊Ø*ùÓÁ@
'ÇÍ3¤ó@ÚP (êZ¿áéÒ­˜¾¿æÜì/œ-{¿ëïée¿ïÿÝbh¢MAGNbcu@'å"h	ԕPowerLawSUMSS J223605-505521?ï؏ýÓCÎ?'pFW[ë;?s¸"¼°Ü?'pFW[ë;?ï4*MÅP?¢ýª×'Óò?™z¶[oˆ?¢ýª×'Óò?íû,½çñZ?
蛝Eo?°&š§1?
蛝Eo?í3cs†¤8?˜qzî=Ü?¶däd8ѽ?˜qzî=Ü?ïÛ~UgÝ×?'æNÑèÌ"?r@ÕCÒu?'æNÑèÌ"?åWs[N?ÒlTû7¡à?ÕQIõcç?ÒlTû7¡à?ìôæòÆd1?¥.ÀŠXºÕ?¸XÈhƒý?¥.ÀŠXºÕ?Õ¼ÏD²rÀ?»T}}%½?å!˜]¦Æ ?»T}}%½MIXED3FGL J2236.3+2829@V†à€øÀ9¢¬_nû`À7ÛAõmÕÆÀ;.ì³òá4?ø¤Z­ Œ¨@Çj²ÑN@5¸ÜU
¿à-Îy—'ü¿ãbºFÊ¿æ·£®à¿èæÜ­ë`6AGNbll@zU4CÔk'LogParabolaB2 2234+28A?ïö;ó"?R:»u×\?Sˆbü'o?R:»u×\?ïÁèV&c}?N,ÉPD?Õ;]@?N,ÉPD?îý¾såø9?—ajø<å? $¿è®m?—ajø<å?ï÷ÃωPÝ?7Р™nÅã?PxacÔ¿?7Р™nÅã?ïâ¶íM±ö?n†	ZûÛÏ?mI¤šQ?n†	ZûÛÏ?ï|(çÍ&?­VÏ/'µÒ?ðzáNL?­VÏ/'µÒ?îãb?¡?<%×_?®Þ®ÁÉä?¡?<%×_?ïôþ¬î¶?OO}'Þ?V¦ÔN©?OO}'ÞAGN3FGL J2236.5-1432@Gñû`^©ÀLßùÐ;À7y#zX‹²À:ÓÔÄ(?ø9ÕÙ滶@ VĹÜZ@#Ì:«¢†¿Û3T
ÑØX¿âQâǓ†¿äZÀþd,¿äØq*\yAGNBLL@'-q²•êLogParabolaPKS 2233-148?ïþ>¤«p‡?/Ÿ`å"`?,µ'$H‡?/Ÿ`å"`?ïÁ¿b"W?™|úê{æ? N㨾?™|úê{æ?ïi€2{Ž?‹"¤?	ˆ?¥Ÿå¢¬t?‹"¤?	ˆ?ïÿòë‰?H>Ь}ÙÕ>Ú)XË…y>Ь}ÙÕ?ïûo£0z?GÅ´;ó¬y?BCî!ƒáp?GÅ´;ó¬y?ïLÉå;Ùu?£<~¸!,?–fÃQ¥™j?£<~¸!,?ïD¹É +?•šôþé+]?—~èÏs?•šôþé+]?ïÿûB"†µ>Äú¯Ÿ™è>ÂøR-FŽ>Äú¯Ÿ™èAGN3FGL J2237.1-3921?âôÕ@"ÀMÌÿ ^¯¹À9§×ÂÊŒÀ;Íiϧr ¿ÙêÍ×lk—@APt6³›@ßß»<¿âCq"öO[¿äF†TËè¿ãèN.Ð稿á@ëæÿ(AGNfsrq@'š篸PowerLawNVSS J223708-392137?ïÿ؃ËbP>ü†3`¢Q>ó¾¹ÈJp>ü†3`¢Q?ïÏ"
…¯?ŽH€íé7?xvnï|®?ŽH€íé7?ï±1¦@F?ˆŸƒÿ®•b?ƒ³–x-Šf?ˆŸƒÿ®•b?ïÿê\Ö_>Õúj¢ƒ‡P>åà'>ù<Œ>Õúj¢ƒ‡P?ïÿñV¼Fº>éuÎ.F5Y>ÝRã¥VÎ>éuÎ.F5Y?ïŒge{0?œã5ÉAî?Œæ&¨ëã?œã5ÉAî?ï­–jvR?‡j=‰Ãû§?"¹Z^ƒ3 ?‡j=‰Ãû§?ïÿ¥>¯Ï?$K—/uÅ?¿gñ÷J?$K—/uÅAGN3FGL J2238.4+5903@Z£h@[9â?ޝ¢ŸŸ›À7±E‡ÉÀ:²›ÉÂ@3¢x:yN@Wúÿ'?þsÆV;¿Ñ–·÷þ~Ì¿ãÈ´˜p¿çìÝÖVÛ¦¿ì›R[ÂsƒPSRPSR@œ_+ŸU›=PLExpCutoffLAT PSR J2238+5903?C^R0zwe?EË¥0¤üZ?ïû(kjBz?EË¥0¤üZ?¡Õ]UuÇ:?»¹Ý–ú6?îâª*q©Í?»¹Ý–ú6?‹hØKcö?'¤²n«?ï'\ -Ì0?'¤²n«?"´ÉË»È?y¾sk¦"?ïbY±¢$?y¾sk¦"?<¨Yht?Í?27€Ž9Ð?ïüjõlÿ?27€Ž9Ð?ŒµXÈá3K?«ûüÛËQÔ?ï*œ¥s?«ûüÛËQÔ?xvºÌ6%?tCÅLÞԄ?ïÏécëô?tCÅLÞԄ?mwü ­êž?`mk«]?ï∀NU?`mk«]PSR3FGL J2240.9+5831@Z¥ƒÑF¿Â8ßowîÀ9•ÝŒ7±GÀ9›V	÷Ї?ú±¯ÀL‹Ê@¼%†¢F?ìêŒèé}¿Ïà'·)ø?»Za»¿ç	'6½›¿ïÿö¯Á›ŽPSRPSR@"©¸7´¢4PLExpCutoffPSR J2240+5832?¼åèÁcÑÐ?ÇN¥
¯Ú½?ìcBçӅÆ?ÇN¥
¯Ú½?é
=ÕÇj?ÑW‹"6?Ë׬¨âY?ÑW‹"6?ÀqÄ!œK¿?ª>W͞
Z?ëãŽ÷˜í?ª>W͞
Z?é ã1_–?µƒ‹?ð£?Ëå|s:©?µƒ‹?ð£?Ä:-k{¬§?Ð>ûO¹s ?êñt¥!Ö?Ð>ûO¹s ?Û% 9,,À?Õ.î<U"'?âm/ãié ?Õ.î<U"'?»$Ï Å:?ª·³¿meJ?ì›fçX®?ª·³¿meJ?áÆc+žib?Åønh_Ý-?Üs9¨Ã-<?Åønh_Ý-MIXED3FGL J2240.9+4121@X‰}ßÿ¯xÀ.Oç_JHÀ:¿k»9ýÀ;|Î>½¿»x'b@敠¼@ž2 f<u¿ã\ûn¿ëT™¡ô~d¿Ôû¤åìÈ/¿á.»c\µ|AGNbll@¤.4êJŒPowerLawB3 2238+410?ïÿ‡NŠÉê?	ÍGŸõÇÒ?,YÄg2ê?	ÍGŸõÇÒ?ïÂdªŠ¾Ç?ŒP8]±º?~ͪªÒhÐ?ŒP8]±º?ïꨌ?'¼?cÁ©()l?eWs£ Œˆ?cÁ©()l?ïø@àè/ ?4Éó_ýÑ[?Nü|o4áï?4Éó_ýÑ[?ïÿ.õ>Ž?Â^ ó+ã?!S'N
z?Â^ ó+ã?î•4ËlX!?²þ2Æ(Ð?¦¬³I:}ø?²þ2Æ(Ð?ïÙüo@™g?v‰eªw?sÈuà^?v‰eªw?ïÄ[Èp`?q½û/'ë?}Ò†ßþ?q½û/'ëAGN3FGL J2241.6-5237@u®6	ÀKuJÞ™À82ª§ÞÖ»À;ný`O@N\Õn@jt#"X?ü‰ïµ…'¿Ð©RÝ{#j¿Ö¦˜"Š'"¿âÚ°E‹-#¿î¸R‰åœ|PSRPSR@L˜"t¼jPLExpCutoffPSR J2241-5236?a7PÌQ¹?vjï­ºr^?ïîÈ°2F?vjï­ºr^?»ÿ§wu#æ?ÉJ\Ú÷\î?ì€[ƒ?ÉJ\Ú÷\î?°È0«€?¢€ÌR°O^?íæý¾9ê?¢€ÌR°O^?ƒ55¦³é?oùŽ£"?ï³+)_°ü?oùŽ£"?héé0çC¾?gùܪ,eA?ïçº$?gùܪ,eA?²¼hI ?ÄUÛbÖ}¿?í¿Hré	L?ÄUÛbÖ}¿?¡¯gíëz?¡8¡ÄüÂà?îåiœž(?¡8¡ÄüÂà?^ýgÕ?YR·u¶/8?ïðù$œ†?YR·u¶/8PSR3FGL J2243.2-3933@vyÏÏÃøÀNW³ S\žÀ:eÄ¿¸TÀ;ð^VÀë~ù°/³@/B%¿W@ò«]ä¿ç—™‡jÿ¿ÝÆLM" ¿è¨šSd¿çj3;°tAGNbcu@Ÿ´¢3œPowerLawNVSS J224326-393353?ïü$ܶØL?AŒS\¾?>Ù1
)Ã?AŒS\¾?ïÙAZp?'KÐEw¸Y?s_Rú7Žï?'KÐEw¸Y?ïo=˽ƒ?†ÚK¤y±?'˜FˆOš?†ÚK¤y±?ïÿü_À©>ÆùáBu>½Þâ7õ€>ÆùáBu?ïïδOõ®?e–ˆŒÎ?`1Kᄱ¬?e–ˆŒÎ?ï<,FC?¯ó¸ó÷À?˜zw8_µ?¯ó¸ó÷À?îžjq7ûš?˜òK8Aø¹?¦Xéªf?˜òK8Aø¹?ïþ×M¦ž\?*©R׈?"‹%3%|R?*©R׈AGN3FGL J2243.4-2541@<t/ ~û‰ÀN±W€•ÓÀ8¨Xçø¢>À;'Ì؋Fð?æƞ‰\Ny@ö˜Ô!Õ¾@2¹@(<¿á²Í¯m7Þ¿ãV'^o¿ä~v"T#¿ê‰2°Î¶ÔAGNbll@‰͞ƒä&PowerLawPKS 2240-260?îÔ+Šê¡–?ÂÝ!%}?¢½GMæJŸ?ÂÝ!%}?ï‰kí @?™q>¶½út?¥'8?™q>¶½út?î¾_µ?šãa½þ?¤—t/»?šãa½þ?íüjõŽ¯?'tó4$%Í?°Ì©e?'tó4$%Í?íƒKu/"?º®¾?§q?³çå£èç?º®¾?§q?ì™=£Ï}?Ã+?ß>Œ?»6á"ö?Ã+?ß>Œ?蛊J¤Ç~?µFÌZE¢ ?͑ÖÕlâ	?µFÌZE¢ ?äëÈ5Ø?¶lϞ'º£?Ö)Àoé"P?¶lϞ'º£AGN3FGL J2243.6-1230@JRe?õ¹UÀL]â?û˜'À:%©|e¬,À;ÁÔ2Ûÿ?Ö®ãû	£@p-è±@ÀÊ+¿äG.B¼Ö¿ì¤"{ó¿¸Pí ‡èu¿ÖãlØ׃AGNbll@¡[hr°!PowerLawRBS 1888?ïÿ€2L*?v'3pÿ?óƒÁz…"?v'3pÿ?ïÃxK|fi?˜Vô×£'‹?~CÚ,7Š?˜Vô×£'‹?ïå:veƒ?n7i
þ?j'nò:¥,?n7i
þ?ïñQžO®5?F".‰"'?]\ÁŸÔÓ?F".‰"'?ïÿ$]'g#?G¤ºÞä€?tS¼¦+?G¤ºÞä€?ï6èÐA)? åy;9¡?™"åôk@N? åy;9¡?ï®hüé?"¥ö‡ ê2?"eÁ%õ?"¥ö‡ ê2?ïÆ>jôÀ‡?qƁ/E·ø?|àʏ>¤'?qƁ/E·øAGN3FGL J2243.9+2021@U¥Â # –À@®(€QÉ÷À7³ŠÁéÀ:žoStò?òý>áß.@QŠDg
*?ü¢Ù;(ö¿Ö"÷ïÃÐW¿Ö'ÇɾᎿÙüÚkÆ̈́¿Õ¢/ÁIòùAGNbll@ ÿ·Ûô‡ýPowerLawRGB J2243+203?ïBnü{ÕÓ?"kmaW]à?—² sôá—?"kmaW]à?îô©S0÷? î"½ËoX? µnéñ	"? î"½ËoX?í#|Ä?´?§päO½…ò?¶ä݆4`?§päO½…ò?íLOøˆ–?"Pù› ¨"?µ€=ñàÕ?"Pù› ¨"?î
ùLÄ?¨Ên¾d
?®.£ÚÏÀ?¨Ên¾d
?êOsxGºT?Äf­!ûl?ÆÂ2á±?Äf­!ûl?ì;\\¢B`?ªb8äu?¾%íí?ªb8äu?暛Ó
aE?¸%(*™ñ(?ÒÊÈYå=v?¸%(*™ñ(AGN3FGL J2244.1+4057@XŸ£ÌhúÀ/"yÞé/À8¤zôŒÀ;?ÜìՁ?êÛBG'þ´@ë¸x¬äû@POŸ¥wH¿Ö¹k:p¿åT|/6µ…¿ã¶C¦üaC¿å'|/Œ›ÀAGNbll@"Ïl¥zxlPowerLawTXS 2241+406?ïÿ]ؚ­¸?å0[?DéžóƒÚ?å0[?ïºxØ¢Ô?•êrR—wa?aÊ…¦ê?•êrR—wa?ïÃn»ZÅ°?{¬}oj¸?~H¢5"e?{¬}oj¸?ïû~ù°/³?%haUÓ~L?B9kN?%haUÓ~L?ïþ¯0bQ?%ÒT—‰Á?%ú._ç?%ÒT—‰Á?îÛEš'¼w?±?Ê¥"?¢K¦U@ƒ'?±?Ê¥"?ï[üN*ìy?¹õA
¦?"€v>Ý?¹õA
¦?ïõÀ§X&»?H/bÇÐq?T~±<t¹´?H/bÇÐqAGN3FGL J2246.2+1547@Túâ€'،ÀBµâ (zÀ9•9"†À;<L$ˑ?çgØx@rP@Ùå_jÉ¢@v9à¡jô¿çy¯nm¿èû#½/²¿Ü'øª˜'Ô¿Í&hä3àqAGNbcu@§ï¢œwškPowerLawNVSS J224604+154437?ïÿl¬Hc?KV¢æXQ?j,®Q?KV¢æXQ?ï¾rF÷éº?–võø·;?€cn;&Y¢?–võø·;?ïí—wwÓ?gÚS·¼?bhˆUR°?gÚS·¼?ï;(?G¶ÈTÒþ?aClعN?G¶ÈTÒþ?ïÿwà>ø?ãë½'?ú&£ª»?ãë½'?îµ>¿áà?¶[¨wäÛ:?¤¯áú?¶[¨wäÛ:?ïÅ//K$Ê?'ý֐^A?}hhJŸg
?'ý֐^A?ïµU5ð?tη©ìh?'¼jµ›¤×?tη©ìhAGN3FGL J2246.7-5205@uFŸŒ!âÀKí: þ¡À:-¼ÎRÀ;ƒìŒ…´à¿Üœ²
™@
½Úg•œ?÷!ÀD(N?ïñA2œ¬Á¿Ý+$Ÿ$P ¿Õ~uh"EA¿³ÔꎺԎAGNbcu@É ·l‹C–PowerLawRBS 1895?ïüc	Sž?AÖR¸‹‹e?<ç³m‰è?AÖR¸‹‹e?ïÒBhÁp´?Œ&@>[Þ?vÞ˺™®?Œ&@>[Þ?ïnsN	?³¦vª_?'1–E¿6h?³¦vª_?ïÿ<Þؒÿ?8~0…è?d)‰.†ç?8~0…è?ïýƒz¸X?6†1
x¤¸?3ä1˅¡(?6†1
x¤¸?ï?*þ~ð?¯B6'Ï?˜ ?P"?¯B6'Ï?taŒô?¯Ïw¨×?š"ÝMï?¯Ïw¨×?ïúò؂Á?=me³1Ð?D4ž€žð?=me³1ÐAGN3FGL J2247.8+4413@Y-÷ µíÀ*€Ô`?ùÀ9¾P"–JZÀ;}ð·Ž?Ö$8'¨T@ "=¼Îþ?üºÊÿm3	¿ä‰?ðcˆ¿ÕŒ¤‰óÅp¿çxíztîÈ?ËÔÁÔiyAGNbll@¶ì™™™šPowerLawNVSS J224753+441317?ïúÔ±êë"?I#B{2¬ª?D­7‡G?I#B{2¬ª?ïºÜΈÊÑ?•ŒÖã]$L?HÌk‹»Ì?•ŒÖã]$L?"aÌ?'ÜÜíßʉ?ˆwuKi\?'ÜÜíßʉ?ïúÅ6¼Ñ?9¥`¼ZÙ»?Dë$Ž1¤^?9¥`¼ZÙ»?ï§L²œ[?mw6I;?†8,É
E?mw6I;?î}>»ìC¤?µe¶Èf|/?¨,A;ź?µe¶Èf|/?î†âZ±/?¡&çÊyíI?§'ÚV¤Ü¬?¡&çÊyíI?ïÂv´´Ÿ|?|ùø Vtp?~Ä¥q2"?|ùø VtpAGN3FGL J2248.6-3235@+}ÿ	_ûÀOué_ªŠƒÀ:ðôÊAØÀ;ñ9F¹?Μhv66@+渱7@"à{*n¿å´ŸzÀKÆ¿êD¼…Vìv¿ënL´cŸb¿ïýðõºÆAGNfsrq@wFGE8ï5PowerLawPKS 2245-328?ïøè2,?VÀ¾ê'?Oˆ_•}ßa?VÀ¾ê'?ïÉÝUþ[²?ˆISòJ©ª?{UoΦ?ˆISòJ©ª?ïFÈ¡nû
?Šô‰'+	?—&ëÓØl¯?Šô‰'+	?ïIYÎþU?{šüzdú?–ݔ°™Y?{šüzdú?ïó㌬Ì&?i»Ô±
?X8æ堂ë?i»Ô±
?îžlȑ?º&²úÇ9™?®Æ÷{¨ì?º&²úÇ9™?ïa=1¹¶?"ùŒ£…äX?œÓØYÈÉ2?"ùŒ£…äX?èAE¢eN?±c
qps?ÎúëvjÉ?±c
qpsAGN3FGL J2250.1+3825@X²à'¤À2']ŒúÀ9(&¶ÂÀ;WD²·wÑ?Á½À´æ|@¬ƒd?þ˜¶?l§s¿å°6E®­I¿ßÁpïg'¿ÞóSãñ›¿Ö2t}xAGNbll@¥Ÿ¡G®{PowerLawB3 2247+381?ïür)=;?2$ý
ÁQç?<n·Ð'ù¦?2$ý
ÁQç?ᄊFxŠU?[Ñ<‹?€RnSo¾?[Ñ<‹?ïعU)ZË?r¸M¿öƒ?s£U\4R¨?r¸M¿öƒ?ïî›ÚøšÂ?L{~Ÿ½C?ad%E>5‹?L{~Ÿ½C?ïî÷Üî«?YéúãD?a$ÏÅ?YéúãD?îÜ9ç­MÖ?­Õ Tûƒ9?¢<a‡¾×•?­Õ Tûƒ9?ï‰Ê‹¡UÈ?\Xϸð?]‰Åö?\Xϸð?ïnG`¼®G?ƒá¡D,±?'7ëÙÓ'?ƒá¡D,±AGN3FGL J2250.3-4206@v"Ÿ×¡<ÀN"¢¿³ÖÀ9½Ì'ãtÀ;À4"\B÷?éž©4'‹@³-QFï~@D– "Hr?î?Þù[\¿à5û×ý,'¿âžì>Ø¿èj'–qñàAGNbcu@™>Åm\ûPowerLawPMN J2250-4206?ïýa+áQ¶?:g#sTÅ?4ö ¦?:g#sTÅ?ïLQ–gÖ?¡(ú'[K{?–uÍ,[7:?¡(ú'[K{?ï¯Ç "ó?ä@¦u4‰?"8±É?ä@¦u4‰?í´}1rØ~?"ÄöJ²?²\saŽ?"ÄöJ²?ïó«yÒ=?gV|48?X©C$Uì?gV|48?냳~О?Ä-`WÐï?Áñ2½‡"?Ä-`WÐï?îÉ«ö‹?žã>¬¢°¦?£cÞÕ@—R?žã>¬¢°¦?åTëÌÐ?´ðûH}v?ÕV)Úf_Ó?´ðûH}vAGN3FGL J2250.7-2806@7½f@¦¹=ÀO§¶€Z-sÀ7ÇtZÏYÀ;[^Ëgr?ï½icà"î@
Ő¡@k(_ššK¿àT¢pN¿¿âûØZœë¿ã õyÐa¾¿å¤ÓFíÿAGNbcu@Œ¦weýŠÛPowerLawPMN J2250-2806?ïÿOÈâ~Ý?š"¯/?äÓJî¢?š"¯/?ïÝxÖà?ƒ"ðá€ÃG?qCþÑ¿¯?ƒ"ðá€ÃG?ï³>l?…쮽®?ƒ:`Lf£?…쮽®?ïý5‹ä5…?"±cB‰¿Ò?6S¢¦Ÿò½?"±cB‰¿Ò?ïþïg_h?(B8±~)w?!	Š2éÔ?(B8±~)w?ï"±u>­?œ<¾N=Ì?Žý¬ÿ(Ê?œ<¾N=Ì?ïtÔ©Ì'ò?;¢\P?'ejÍZ9¨?;¢\P?ïûÛ®šB?7oŸÔ*W?@'E?o.?7oŸÔ*WAGN3FGL J2251.5-4928@uJ^`=WyÀLú`à¨.À9³C½Äò
À;¶V¼¥7]?îyù$]q9@©;"@?ÿx®àR»¿âzï(‹¿ÜSLÙ!š¿Ô§RR:èè¿ä%ržê!®AGNbcu@ŸÆ¶âëCPowerLawSUMSS J225128-492912?ïõRtcv"?UÔÿõcÜÙ?U[œ–Ð?UÔÿõcÜÙ?ïiMzBw…?"]÷6j»¯?'ÖP¾GV?"]÷6j»¯?蘆®µ?Ñģħ?†Ò"Œê^®?Ñģħ?íð"]ëB¯?‹¶1½­Ä ?°{eïÅ	?‹¶1½­Ä ?ïåúÇB/Œ?k`ªW\~J?j8˜´¬™?k`ªW\~J?éŒèe{ý?ÈBÃÖÑð?ÉÌ^jˆ?ÈBÃÖÑð?ï&" á.?˜2MNDT?ž;ª,C?˜2MNDT?æôG•û?² Mz͟²?ÒÓpÕÖ?² Mz͟²AGN3FGL J2251.9+4031@Xè#¿ø¨ôÀ0àé_ªŠƒÀ9:$)ªô5À;‡Æßî¿ÓH:õR¸@Iá">éu@þh`f¿äÊD;œ<¿äW§¢¬ùÚ¿ÙéO¹?–¿éí'u¡ÓáAGNbll@"I°£×
=PowerLawMG4 J225201+4030?ïñVàȓh?Y[¬ù€?]R>¥Òîí?Y[¬ù€?ï½½΍?'6ÚW~?€ 9,"¶?'6ÚW~?ïÖšÚ?‡¬1ئ¶?‹ÊYnÊý¯?‡¬1ئ¶?ïòŠkÔ9~?Eý·-"û?Zë(eKt£?Eý·-"û?ï¹~´;?€ä$Ïç.? RôVB?€ä$Ïç.?îÛeñ˜Ös?±1ÄQ¶Ó}?¢I ær˜×?±1ÄQ¶Ó}?ì،ŽnBS?ªk•/`?¹;›Šh+ì?ªk•/`?ïæwBז?ƒ†÷ò'?†b(jâŠ?ƒ†÷ò'AGN3FGL J2254.0+1608@U‡Å_ñ_ÀC_ÏspÀ4ƒJïèZÈÀ9ñ´Ï€t@7PÜfs@&LÉn¯?ÿ¢F…‰A¿áÀìªkV™¿ædˆ­ZŽ
¿æ˽ eí¿ë§òX*A%AGNFSRQ@yËóš¿PLSuperExpCutoff3C 454.3?éo~í¾+l?ÑÏÛ¹¾?ÊBIRQ?ÑÏÛ¹¾?ïÀ®ë\?œ•ùoû¸?ý(œÅµº?œ•ùoû¸?á­h¾c?µ˜üUi?Ü¥ý.ƒ9ö?µ˜üUi?ïÿù^ówÔ>ËU*>ʄCKìF¨>ËU*?èÌyþý)??Ê(sfª?ÌÎ[?Ê(sfª?îò©x+W?·6õÚiä? ×kÿ‰?·6õÚiä?æC?åjŸÓ?¹Sçë ?Óy€5*ÀY?¹Sçë ?ïÿÿhš7>¡Y¼5>'í¨øîΑ>¡Y¼5AGN3FGL J2254.0+1403@U'‹ŸÛÒúÀCõrØœÀ:0<îÀ;aC§õ|ï¿àõÖã?ïž@Uö÷Îÿ@ì‹àžeÜ¿æ4»ÚåÄ¿èÖN+î+¨¿áô%öø¬¿É#ò)ŽÖAGNbll@¤9¯Ÿ¾wPowerLawNVSS J225354+140439?ïÿ³XÔÏÈ?}¹øÍI?)Ì՟q?}¹øÍI?ïÑwïÜ?ŒQ2Äð¬È?wÄë
?ŒQ2Äð¬È?ïî–8f"õ?__Ü4Lüq?aiNJ¾Ãs?__Ü4Lüq?ïÿ·dýýê>ô¶(ÙtÀ:?&¹$f®>ô¶(ÙtÀ:?ïÿ¶…òÀ?\a¦½U?^ÁWFž?\a¦½U?ï'öv"[í?®ñʨI$?›12›ìW?®ñʨI$?ïÊq®¡œ%?tú½È»W?zÇ(юD?tú½È»W?ïý}0…À?/=Uo0"›?4"ÿc¨U?/=Uo0"›AGN3FGL J2255.1+2411@Væ æÀ?ƒ:€.Ž‰À9_h-æÃÀ;€·Á¢Í¿Ób:h—Õ0@Œ—[Pޕ@'ž‡t©¿Þ€ÔñßUæ¿ÏÁô—1›¿æ:'Dˆ¿Ú™ó¿ˆt6AGNbll@¢FŸ|í'hPowerLawMG3 J225517+2409?ïÿ¤?•?Qß/'ð?à8cÄé?Qß/'ð?ïÖ)Ókªü?ƒõ´|
â€?të?Û­Ó?ƒõ´|
â€?יּúb1M?'e‡ž¨Î?"сgs¬ ?'e‡ž¨Î?ïÿ$[æ?c'"Œ¨?t{Z‹J"?c'"Œ¨?ïÿ9yx6?>ÅÜëA?ÐÖ¨²jí?>ÅÜëA?ï¦Ë±CÚ?²=¹¿–é?«&ˆ¶¹?²=¹¿–é?ïeèO'Âî?Ž½'H÷¨‰?"Bö>0?Ž½'H÷¨‰?ïùµSš˜?BÓP0ÜL?K)­-?BÓP0ÜLAGN3FGL J2256.7-1022@M›Ö_ó…žÀMCÀI0ËÀ9˜OYÚféÀ;à,/2ór?ü
߬ùH@¸åå!­?ùrLK:\?íN'˜Œ¿×lôS¾1î¿æ&äv?U¿íšpÙÃPSRPSR@'Çì1&éPLExpCutoffPSR J2256-1024?o+ÎÝ?®?|Þðg8úÅ?ïàpÔ1"À?|Þðg8úÅ? Öéuë?ÍÎ!°Ï?ëwÊE¢»E?ÍÎ!°Ï?Ë61{‰I|?°‹¾©bSK?é2s¡­¡?°‹¾©bSK?¬òðÞ0Ç?R}m—qÇ?î0Ðò@T?R}m—qÇ?cÓ[¯Á?b»_Òª?ïì,¥
Í?b»_Òª?µÝ†äxIš?ʏ'x"á?íDO#9ý
?ʏ'x"á?¸Ð‹ˆFÑo?§¼ñ="‹?ìåîŽégb?§¼ñ="‹?{¶Œí¯]‹?ijl¦ó?ïȒåí§…?ijl¦óPSR3FGL J2256.7-2011@DÈL€SÀOt?Àà0À9HÄIpŒZÀ;—¢çöô¿¿âíÐ.q~@
/óf¿|­@½}ÿµ,r¿Ý}Ì¢8,J¿ã[úk…¿ßp÷TñÛ
¿ä¹±~AGNbll@•šu%PowerLawPKS 2254-204?ïú'ßÔ"?F¼Âz›ð?G"`E҂?F¼Âz›ð?ï×	駓?"Û–ü÷°þ?t}û'Yv?"Û–ü÷°þ?S|Â?';†ºTP?‰kÌ'?';†ºTP?ïõd"V‹?EI bÿ‡=?U6ÖvÞÊv?EI bÿ‡=?ïêà·ÌpÃ?g£³1=?eHQËÍ:?g£³1=?ï4Ê US!?¤qÏÝð­õ?™f«õU›Ø?¤qÏÝð­õ?î〗¹?–À™&jC?¡ÇþúÏòû?–À™&jC?ïiÊӒ'¤?ˆàÉ?'Æ¥'*§w?ˆàÉAGN3FGL J2258.0-2759@8ZÝßCÇÖÀP:B×P´À7¾Éãä@‡À;=ĵ§Z@'ûE[(ñ@Þ%™Â‰R@øӞM2Ž¿à¾o'Þ9\¿æ—ò_®fZ¿ç:c‡Jë¿íD¿ÇžPAGNfsrq@y…‡"ݘLogParabolaPKS 2255-282?ïͤ—¾;ÿ?Œ8ô²&Ö?y-´AÞ@@?Œ8ô²&Ö?ïÏIx]΁?ƒÓ­nê?x[Càæó\?ƒÓ­nê?ë+µvUŒ?¯·Üäg¶,?ÃQ+æ&©Ò?¯·Üäg¶,?cñ3*ò?k¢Ù•'?€Ÿ©>e‰?k¢Ù•'?ï·Óã¹Å«?³y E&p?'Õ5?³y E&p?ï<—zQø?¯Äñ±©‡?˜m°™"Ï?¯Äñ±©‡?íÆÕ:ô6?¤ûWž©L5?±ÉV'q?¤ûWž©L5?ï¶X3ȯ\?zî
«	'?'ió¢\÷?zî
«	'AGN3FGL J2258.1-8248@s04ÿ†]}À@³€ KÏâÀ9‹pd*À;vx†?Ò±ó¸Ê@ÏZs@ŒóŸŸm¿£q³üª¿áÙþú±7¿à&Ì¢Qñ\¿èUj3`»¾AGNbcu@XU$ÝPowerLawPMN J2258-8246?ï÷‰ˆ÷­C?UÊù·1G/?PìînÚ^?UÊù·1G/?ï»f±ÿ†?"t=#'öŠ?8¦J'"š?"t=#'öŠ?ï»îœo&?|íz"‹/Ñ?8DK%Æ£?|íz"‹/Ñ?ï®ÁBVö?d!ôz_õ?"O¯±Ô_?d!ôz_õ?ïèEPíw?kÙ5×£x"?gº®ìèâ?kÙ5×£x"?î€ß¦Á?·jéÎm?§òL!Y?·jéÎm?îák¤áÕ?w.°x ~?¡éE´'7¯?w.°x ~?í° ®¸~?•oß9u'_?²~ÿ'Š<?•oß9u'_AGN3FGL J2258.3-5526@t®÷_²íþÀK'¡ ÏÀ:zi
à"SÀ<ë7@?ÑòG" S@Ò3>íÂ@|®¸'¿æŒà/¿ç[î¤ý"°¿éÝ=K˜?»°fQvHAGNbll@"ÒÜàuöýPowerLawPMN J2258-5526?ïü)È6¡8?D¬§¸OøÓ?>±Àbl&?D¬§¸OøÓ?ïÉvÌ:*É?õ›™Ã?{D™ëٗ]?õ›™Ã?ï@r‹ã£?…UÜ/µ2#?Œ¯ã`v³?…UÜ/µ2#?ïùnÅ>'?>~¥'Í?JG¸ãU?>~¥'Í?ïá|È08‹?|Gבk1°?nƒ7ÊHt?|Gבk1°?îî]fô'ô?µ¬²¾î7¸?¡)¶àÁ?µ¬²¾î7¸?îx¼z*z?žóy!!Ì?¨v$8]Xe?žóy!!Ì?ïB½Ä?‹õðìî?Œ/P±‰º?‹õðìîAGN3FGL J2300.3+3136@X5 "ÚÀ9
¿v¢õÀ9Eˍ1¬JÀ;df\Ukl?òˆ–i¹W$@¯¼EÀÿ?ý™ž>ÄáÇ¿ãŸM›lC¿Ì-H"÷Ò¿Õ-	²u!"¿ã~bª€WåAGNbll@¥^Ñ·PowerLawNVSS J230022+313703?ïó›Žnö¶?U‹µùG9?XÈã|ÈBÆ?U‹µùG9?ï`™š?œQîgÚ¸P?"ìßÀ.(¾?œQîgÚ¸P?i•+1?ˆÚ"}?嚵3º?ˆÚ"}?î"Ä—8B?€˜R¬Ö#l?§³¶‹£Ôß?€˜R¬Ö#l?ïàûÀ«+g?pMôÕÍ)?o?(٘Û?pMôÕÍ)?ìØ&ž¿4?ºn:g¯è?¹>Ë	™ªã?ºn:g¯è?î—Ç÷RX?ž=KPe'?¦ƒ€"s?ž=KPe'?ëR2AÆR?¤ü"3,?·7âøæº?¤ü"3,AGN3FGL J2301.2+5853@[Fú>¯h¿ï'DŸÀ9Á¾òïvEÀ;:9%»{l?ò³ç®O‰*@åÆî¼a?ø7¥þ׶á¿Öæê…Dwÿ?ïþzÄÂ<P¿ØŸa´ü¿×Á›@bÇOTHERsnr@Çíê^5?}PowerLawCTB 109?î¾×M¦ž\?½þÿ±ÈÜË?¤‹#e??½þÿ±ÈÜË?íyI²Ñy?ºýÛR_?´5²g¼iã?ºýÛR_?î5÷¥µÔ?^SûÞ:ç?¬ …¦Z¹?^SûÞ:ç?í?aÅ fE?—Ó(MÕ`?¶ñÒüÍØ?—Ó(MÕ`?îCܕºq?­¾œrçÔ?«Â6¨ªûä?­¾œrçÔ?å9f€4I?ÐE2®:?Ս2ÿ—áo?ÐE2®:?ëÍOeæ0C?¬Öð?­9ë?ÀÊÂhg>ö?¬Öð?­9ë?禕٤)H?µÒzl\és?вÔL·­p?µÒzl\ésAGN3FGL J2302.7+4443@YÙN wmÀ+ù¿è,À7ý£ª"" À;L(T²ß¼@-ù압@h´Is<?ú'òg»ü¿©ÿP¶.ƒT¿×ÿ'¶•B¿âs~õõ¿ìß²ÔPSRPSR@¸ÐË)^žPLExpCutoffPSR J2302+4442?U¼ö£e?V':ïy¦Þ?ïõ!…
ìB?V':ïy¦Þ?© aÜö"?À¹ËÂz}8?îmùï´r'?À¹ËÂz}8?›ük|ÎþB?":V'Qä‰?ï ¤ɞ?":V'Qä‰?ȗŽÁM
?au'Ó8`Á?ïÔfÜØÞ~?au'Ó8`Á?YþŒÿ—?Qí¿èz²?ïó¹Ae?Qí¿èz²?ˆ-êQZ?žB;"/?Hœ¦ê?žB;"/?"†šnÄÄ?€¯5"¹Ä?﯁åjIí?€¯5"¹Ä?PFªê^*=?F¡¾'¢¹?ï÷ܪ‡ÊÜ?F¡¾'¢¹PSR3FGL J2304.6+3704@Y^"ñÀ5"ÿÖåUÀ9q¬'$ZÀ;iQÝBeÖ?Ýí¾jŁæ@¤Ô…'ò?ýÀŸ¿äm½å ¥Ÿ¿çÇ"5¿ÌèZ²Ì¿²<´fN"ŒAGNbll@±d"Š	PowerLaw1RXS J230437.1+370506?ïâßKˆL?­èHç?m ´läóË?­èHç?ïɽög@?"®•úß¡ê?{!ÐPè3?"®•úß¡ê?ïï¿í…ñ?gö)lè²?`@b*Þû?gö)lè²?ïúÂSw s?-ä¨,w·?Dö²$
ñ/?-ä¨,w·?ïþRšõ²?/™üûã?*Ö_ђ›?/™üûã?îÈ,¨eËr?µ%ˆ@Nü?£}5y£Hß?µ%ˆ@Nü?ïÖ?àh?~ZjHŒû?tàDUó¼?~ZjHŒû?ïì1j
î?W˜4"ãõH?côΈ3¡µ?W˜4"ãõHAGN3FGL J2305.3-4219@uîCÀ~à±ÀOÎ*ŸæºµÀ:ßNG‹¯ÌÀ<]û]Ùпê/wAÞzR@
¹µ.Ëo€@b¿g£¿í ›:¥å¥¿ /-¥ l¿åoº 9¿Ú]2p?®AGNbcu@¤î¾ß¤@PowerLawSUMSS J230512-421859?ïýbf|‹Â?@¸­Û‡I?4ìʈ¡?@¸­Û‡I?ïËqØ.?ê)Åob?z~G&"Ì÷?ê)Åob?iløs?'Õž|µ6É?‹•eµïï?'Õž|µ6É?ïþìÎ?B¾L ?!8¦eæÅ?B¾L ?ïô5n̼\?^ÓAVœ¥?W•"@¨¿?^ÓAVœ¥?ïPàû'í±?©¿,΅­«?•ãàŠzßô?©¿,΅­«?ï'höÓJY?'ìßø·¡?›á*¾Ó?'ìßø·¡?ïì´lP-?`4—˜TÎx?cúKˆ±Z?`4—˜TÎxAGN3FGL J2307.4-1208@Mµ?Àà0ÀN±v_Ø­¬À:‡kþUÛÕÀ;Ç%l¡¿Üø'y'Å@q!Ôæ÷›?üXFÀ®±Y?è@wO€¿åFðqdÆ¿èC,f ¬"?áQoß6öAGNbll@²i2£S&PowerLaw1RXS J230722.5-120520?ïõm>Ù?°L8§Ï,ò?~%pPﷁ?°L8§Ï,ò?ïՈr!R?'8Ï՗Øî?u;ÆýÅ[?'8Ï՗Øî?ï
!ŽpÅ?':ßBþÕ?ž[Î5lCV?':ßBþÕ?ïÿ¥bá²É?÷"öã(?§F:"€?÷"öã(?ïòZb!2?cuW9ªö?[óKž²ZÍ?cuW9ªö?ï_.zÖy¹? ý=,+8/?"0¬ä? ý=,+8/?í¤œ[ã"?¥×÷õ°Ì?²Û!ÂÖ%?¥×÷õ°Ì?ïøŸcæÀ?R·Â¿^Z?MƒºŒnš¾?R·Â¿^ZAGN3FGL J2307.7+1449@V5X`fÀDŠæü9¢À9ñÝ'ŽÀ;gÝX5K;?Ï$¢v·íB@lÏ$ÀԜ@èj#ç;¿â}ˆŠ¿â˜@URb¿ä¾Æ³>lˆ¿Û³ÝF[rÜAGNbll@"Õà[À7PowerLawMG1 J230734+1449?ïù¤'oS ?G"ëhbë"?Im¹Ø
mÌ?G"ëhbë"?ïÇPB0Z?¨ÍÀÇî²?|W¸=;§M?¨ÍÀÇî²?ïS¥Í@?Š©-7%.?‹BîÛù?Š©-7%.?ïϦ"I•Ã?a©)ÚnöÙ?x,¶PæJÃ?a©)ÚnöÙ?ïÕXwV?z6yV]¥½?uSû¥‰Y3?z6yV]¥½?ï[<øÀ?§Û'"?ši?t˜bŸÍß?§Û'"?ši?îûid¿ë?£Ö@£e²?¯ Ieh~]?£Ö@£e²?îú˜{Ñ!?üÔÁ'?¯VxBí÷?üÔÁ'AGN3FGL J2309.6-3633@Cï@j(hÀP ½_ÜßjÀ9øÀysžÀ;­›÷Aë]¿ñsCÄzï@]¸šºx?ý«¢¥é¿é«FuÔG¿âÚ2ÚKæ¿Éð'ék¿âD.ŒÊ*AGNbcu@¨	ØFÜ]PowerLaw1RXS J230940.6-363241?ïþÜs!Ïw?%J†'Þ¯ ?"8ËÎÞ¦?%J†'Þ¯ ?ïÜ¡YèÝ?…Ò²Bqp?q¯SHu{?…Ò²Bqp?ï§ä<¢j?Œ²·…aâ?†ðÓõÝ~?Œ²·…aâ?ïÿÔ@UýÛ>ñõû@ƒÑb>õß½rxŸ¨>ñõû@ƒÑb?ïÿ‰'Ü?ƒCÅÙ­?®ÆößU"?ƒCÅÙ­?ï"}übÅ%?  ½Bsˇ?Žà€çN¶Ð?  ½Bsˇ?ï¼d??…fOF7"?€ûºIµ$=?…fOF7"?ïþÙ/ÂÌ? ®Ò$Õ?"mBÿ+p? ®Ò$ÕAGN3FGL J2311.0+3425@YPaAcxÀ8_€™"À7‹áP°À;&ûL<µ?ûz9.Êó@3¼]éÀ#@㶿á™üL[7¿åWʯï¤ò¿åY‡lÀV¿ëÌkŸÐRAGNFSRQ@w	"[l7aLogParabolaB2 2308+34?ïæé §?dŸî"À
n?iÿå5é1?dŸî"À
n?ï¾'˜þ¶?–©ÿt=4V?€v?'‰$l?–©ÿt=4V?íÚiÞà¡?£)ÜI î(?±,·™äáú?£)ÜI î(?ïýçþÆ2ï?†1Úù?0À	Ê9¯?†1Úù?殮&S¬?"áqP½z?†V¶†i…
?"áqP½z?îî°ÔQY?´«¡í-Èï?¡"ó–Ñm?´«¡í-Èï?í1j¬NÜ?§Ü¦ýèi?¶sôª‰$?§Ü¦ýèi?ïþt©…A?&	Büã'?(·ä–ê}?&	Büã'AGN3FGL J2311.0+0204@SÔúÿåþÍÀJ
@TƒæÀ9ÜàáVǍÀ;Æ)}§ËŒ¿ô
ý\aªÀ@d¿o—ª@+b€R˪¿Àâô:"¾}¿æÕÝCßË$¿æ˜	Œú¿Ï¯7¼AGNbll@' ¸ºÇPowerLawNVSS J231101+020504?ï
ÓäTd?ÄsLl®î¯?œžE~N	"?ÄsLl®î¯?W3‡?˜z†j#?~¸¤oã,?˜z†j#?ﲆõýó‹?ƒÑ$(è"?ƒ^B‰r?ƒÑ$(è"?ïÿööŸŒ«>Ìié³$SÔ>Òu€‰G>Ìié³$SÔ?ïþÉpe²{?3³eÔðY?#hü \֟?3³eÔðY?ï>Æu€ò?´ÒÙ[Ýhª?ž˜'4¿}Ã?´ÒÙ[Ýhª?ïáӀVc?šq]ê8O?œŏõ3§?šq]ê8O?ïÿ‡þS—?v¥?ö0?ŠŠÝ6?v¥?ö0AGN3FGL J2312.9-6923@s¯£¿ø¨ôÀF®v?ø="À:Ë-œ}ZÀ<	،°?ã›U"Iƒà@
^,±
ÿ?üÝK?nå¿ïÿù?Ð??ïþÔè‹Uo¿°œ§W¿ä8tƒ4¨SAGNbcu@³}Ú¬1PowerLawSUMSS J231347-692332?ïý:{¯k?6€ÿɄ T?6,$[¥kÆ?6€ÿɄ T?ÙQÚ?"o$«É?‰>Sú]g?"o$«É?ïÈ㥮?wï]ó\¢Ó?{Ž-'פ¯?wï]ó\¢Ó?ïd\~?"!¤šõ~c?œ_ómö4?"!¤šõ~c?ïùwùòÛæ?I]‹p´[?J RŽG?I]‹p´[?í~½e¯9ò?»zñµd?´
ÓÐ
ë?»zñµd?ï"ú¬6²Í?†Ülä$?‹Tü¢ ¨?†Ülä$?ìÍÁ?§Ù?¬åB€×K™?¹'ö	¢8?¬åB€×K™AGN3FGL J2314.0+1443@V¡ùŸÿhÀD÷"ßÎ1QÀ9Ž—rwì¡À;f"Ú<ø¿ðÃðBÛ@Ýá"êµì?ü \†ã‰¿'îâ:6 '¿Ôa÷8R¤¿ßï§yu¿¥Šòóä$AGNbll@³`¸QìPowerLawRGB J2313+147?ïý¦BÃo?3xû¢hœ?2Íðøþ"?3xû¢hœ?ïԌs/;q?† •6]Š?u¹Ær±˜?† •6]Š?ïѯ5ÉKÊ?r¨ÒÙk•Ÿ?w(e)Šã?r¨ÒÙk•Ÿ?ïÿßE@Ï>霥ù>ð]‰%lÃZ>霥ù?ïúâ´À'€?H½*ç=Ó?Du,!í®?H½*ç=Ó?ï;$Ä/šL?®ãYb94?˜›gqu°~?®ãYb94?ïŒ#öÁú?ŒþÏ;W"?Œ÷8Ó}l?ŒþÏ;W"?ïþ|Ÿãµ?&ß ƒßK?(6Öü~Þ?&ß ƒßKAGN3FGL J2315.7-5018@tê ßÞøHÀNAY@
6IÀ9»˜"à5À;Êd¨ E?å1®v©S@
ÀXr‡ÜÙ@†@.l?ï+šeÏñ"¿ÞtXÔ¤ÔÙ¿åmÊ"Dñ¿ëÒºŠUAGNbll@"ÈÑÎ_PowerLawPKS 2312-505?é53c.Îu?Å…Vc€?Ë+2sDÆ.?Å…Vc€?í¾©4'‹?·tÆM:"?²
¶]Ù.?·tÆM:"?ërÊ
áÁ?¨sÀª—¨?Â4×ÔxùÍ?¨sÀª—¨?ꝁq?ïj?§¦»I¬A?'nú;BV?§¦»I¬A?à$¡þv?ÍSOýˆ?ßÿ˶¼?ÍSOýˆ?åh†'¡Á—?њ"‰Í9?Õ.òú¼|Ñ?њ"‰Í9?è7ïìž?²T×5Xê?υ‹ @M‰?²T×5Xê?Õ¥;ñ?¸^uÿ¾h?å-}7ýâ?¸^uÿ¾hMIXED3FGL J2316.8-5209@t¼]ÿÅGÀM«t`$-À:£\ŸTÀ;ޏ±¹K¿è i6ÐK²@jîªB3V?ûÂ@&¿èó(!öñ¿å
m*È"¿Æ<C_½r¿Ö§kŸ‹KAGNbcu@·¦?PowerLawSUMSS J231701-521003?ïÿ†I'3?;-YÜÀ?O2}ÿM?;-YÜÀ?ïË5²á¶‹?'

<Wô?ze&s§Ú‰?'

<Wô?ïà:…ëoƒ?ma¾'Ë•?oÅyÞö•}?ma¾'Ë•?ïÿ`Á>Î?nÕ}å?çÑ6*Ó]?nÕ}å?ïÿ;¸–¸?AiÛ?ˆü9îst?AiÛ?ïTR'ƒÓ_?¯72øV?•u¯­ÍÆ+?¯72øV?ïÞÊÎùUu?q7Ëcå.?pš˜†Äá¹?q7Ëcå.?ïùq(Øð?Fë¨JÓ®L?J;"¦AA?Fë¨JÓ®LAGN3FGL J2317.3-4534@ua›«–òÀOà§`+¹ÂÀ9kÝ3L]§À;²ýî­È¿Ê$Û
ŸÀ@â%¯çä«@}1ÿò¿å"¸#G'Ë¿ä5wãˆÈ]¿×iØM€Þ¯¿åD;8?SAGNbcu@'ŒwéùrPowerLaw1RXS J231733.0-453348?ïþ@)]>?09ž8ñ=?.ùƒÐÙì?09ž8ñ=?ïÍ×TÌFP?'lN6ca?yU~?å?'lN6ca?ïèKSœ€?g=´Ú}e?g´¬¯ÊØ1?g=´Ú}e?ïù	=\?6ù;¨LÌ[?KÛ"<Öñ?6ù;¨LÌ[?ïþ€à wÖ?,+ŽM˜›F?'ñûÉõX0?,+ŽM˜›F?ï+«®³Ëä?°5H°üj?šŠŠ&çŽ?°5H°üj?ïÅã 4#¯?13ù\šÜ?}/ø|E?13ù\šÜ?ïÊÊ%cÎ?lñåEK?zý›û"ë?lñåEKAGN3FGL J2318.6+1912@W£?ãDÞÀC?N™À9ÍS¿šµÀ;´¢Þ¼¹Y?à}Ç2÷v@	(ô@P@íÊà
œK¿èǚ´Tc¿èMÎɍc¿èúœQÀù¿ïþŸûˆwAGNbcu@{ç ù	lPowerLawTXS 2315+189?ïóT>#YÕ?bìÝ^ûn?YW"/~å?bìÝ^ûn?vÙâE?†ÔQdï?ŠbFÒµ?†ÔQdï?ïg  "?3Há¬?"ëþGA~?3Há¬?îO7¶?‡G@æ?«nŸô;L?‡G@æ?ïÚ÷¬ìª?v_†Â>?r")'Ùé?v_†Â>?ëø#Wö¡?Á;M$UÁ?Àr¡ˆ%~?Á;M$UÁ?î¼W­°?™ÆFiԁ?¤:…+áJ×?™ÆFiԁ?ã¦ã{‡W?±µìŸEÃ?Ùܲ9ñQ?±µìŸEÃAGN3FGL J2319.2-4207@uÆ# ƒ˜¦ÀP|Ù ,Æ2À:7_èžÀ;âØ+¥ 8¿çG²,s¸@g0¨êD'@¾àP]¿Ó&(;f3¿æ,u
Ü¿ß|c0"ŠÇ¿Õ?\hØþ×AGNbll@Ÿ2a|ÚPowerLawPKS 2316-423?ïÿƒéâà?
OAH¼)?vìÜp?
OAH¼)?ïׇ2}£?†qiۓ?t<rìðzo?†qiۓ?ïà³üh¾'?p}éÒ!Ž†?oL"') ?p}éÒ!Ž†?ïÿN—g»%?‰Ü,6"?-dÙ?‰Ü,6"?ïÿ•U"'r?7'J€?
ª´KB5Ÿ?7'J€?ï^ÄÅÜ•?¦íöpz?"'g?WÃ[?¦íöpz?ïÙŸ‰ü ?uÕYµ¿DB?s|°eˆ?uÕYµ¿DB?ïø#i;?D2"·Êð?Os¦Åd6x?D2"·ÊðAGN3FGL J2321.2-6439@sځ¿½ð'ÀHç( 2:À:ªößÅÍÕÀ<	ø¶_¢þ?Ù+ÿY´H¿@'¨ÀSÓ@4ôBp¿é§ÇQ/?¿çªyW@¿Ùù¼ÚçB¿á>ãAAGNbcu@'úáG®PowerLawPMN J2321-6438?ïþïƒÓV ?ªpEï† ?!Åóۑ>?ªpEï† ?ïÇÇÆ8ð?ŽÂˌÈà5?|×)Y¯?ŽÂˌÈà5?ïÐ÷èÝF?y†ønôyï?w"vœ|â?y†ønôyï?ïÖۏz?XÞ`
"?*?tñT%ÿ?XÞ`
"?*?ïý!»ˆú?7Nä5¿j'?6ò#®J…6?7Nä5¿j'?î®úµ¤xV?±¹î—°‡Þ?¥T¤Ü" ?±¹î—°‡Þ?ïY^ãK"?Ý\Ÿº±F?"Ô=Þ¿x?Ý\Ÿº±F?îÏiR\¡Ê?'~ÏÉuL?£	jÜɘ[?'~ÏÉuLAGN3FGL J2321.6+4438@Z¤[0HÀ.»›>µGuÀ:ýþž1À;ºÏ' =¿ÚRqÿn,%@k¢Câ-@ÿYfú¿ç¯3ëáæ¿ì8æv1Æ¿ÛId祿ïÿŽî½AGNfsrq@~•çÀn¹PowerLawB3 2319+444?ïþUbsu?-ôˆyî(?*©ÛqËй?-ôˆyî(?ïËpÿÉÇ?ˆ'Y6'.m?zGø!\}?ˆ'Y6'.m?ïÿo?­?{BÛ­÷ZÑ?€$:h¶?{BÛ­÷ZÑ?ïóqUœƒs?Dö³xWrŠ?YT@Hkf?Dö³xWrŠ?ïÿøÝT?#Ö%*üÁÔ? äi`
?#Ö%*üÁÔ?î—iãbT?µ!]Œÿօ?¦Ž©^Z>À?µ!]Œÿօ?ïPØY6ÁÍ?ûçùk>Ò?•äôàþ[?ûçùk>Ò?ï{"iÑÑ?…PBê^£¼?›²Àµ{ó?…PBê^£¼AGN3FGL J2321.9+2732@Xêãÿï9À?A§¿Í
	À9bCá× 
À;¢d¾£À	/]k!Ð@Hÿnàˆk@BPàW`¿å']竏)¿â's%Ui¿ã˜|+RFÒ¿â	&I{RAGNfsrq@¶W
=p¤PowerLaw4C +27.50?ïý{çé?2qu¬o½Â?4 ÀõãC—?2qu¬o½Â?ïލ累 ?zºªS¯¹C?p¹*L?zºªS¯¹C?ïʍyÈp?tMœ?z¹CøGê?tMœ?ïÿÿtóO¡>›RB'#b>'YÛË×£º>›RB'#b?ïöö½ÏÉ?TШu¾ÁÇ?R…jlî0?TШu¾ÁÇ?ïBÞz°[Ž?®qÆ	ݛ?—¤0¦"ò??®qÆ	ݛ?ïG9ƒ?—•x·F´¸?ž—Ö}µ?—•x·F´¸?ïÿæ¤ì´>÷z—<Þd>éæŒÔ
.u>÷z—<ÞdAGN3FGL J2321.9+3204@YkìAÝ"À;àÿ‰¸{À8«ˆTüÀ;j´MzV?öØïæ|,@9DQáõ@,n;òÊb¿Ø›£¯¿ä%:cËxÜ¿ä˜1&éxÕ¿é,ÛGÁœAGNfsrq@'h{_ïJLogParabolaB2 2319+31?ï󎇗¹?[ˆ¹rk:?YÔâoŸ=Ô?[ˆ¹rk:?ï¶#[µïw?™ô»§%ê?'w) B'7?™ô»§%ê?îìšò×oà?—þb€"ž?¡6PÕøö?—þb€"ž?ïìx4€K{?GD)Ê|Ò8?c‡ËªO¬¶?GD)Ê|Ò8?ïÌÂÖ U?z'b
V.,?yž"ø1?z'b
V.,?îþ+WOOÒ?²$áäX? JˆwMã?²$áäX?ëh3(²Œì?±»½)ól¿?Â_3]5ÌQ?±»½)ól¿?ïݳûMFb?d[0¥&Ò?q&k겯?d[0¥&ÒAGN3FGL J2322.5+3436@Y·ÃŸý`éÀ8ÇóÀVœÅÀ9þæªÄdHÀ;v zÉʺ?çS¬#xÄÒ@"DvÒoN?÷­ µT?Ñi-竹¿êAb7­–¿ÐE­e¡¿'ãžSbAGNbll@Ï©xÔýôPowerLawTXS 2320+343?ïþª«e?7Pø6ô[D?.~D˜,Q?7Pø6ô[D?ï¼jYe!?'¯A5ON9?€åi¨Ç~>?'¯A5ON9?¼ò0¬?‹Su³?‰™Ð²EÉ?‹Su³?ïØÃÙDr?_ìK/bÊú?sžŒ[æÙ?_ìK/bÊú?ïý‡Žîà?>$c¦"?7Ã2ÿ?>$c¦"?î¤Ôûfà?²ýH½‰!?¥²°F"[ò?²ýH½‰!?ï}ýëÂu?^­°3?@BŒØÆ?^­°3?ï<1tŸÂ±?\f&›?˜yÑq/Õ?\f&›AGN3FGL J2322.9-4917@tè¶@c^ÀOÏ`%ÆÀ9Ïûf=K»À;¨Ø+¥ 8?æD`ؐ'ø@lõÌ ?ÿPý Q¯?ïýÆÖØX5¿à'ÞIvìq¿ß̃ˆ©¿âOuiõ£AAGNbcu@¨k…¸RPowerLawSUMSS J232254-491629?ïýD/@³?54jÈæ?5ޅ"1ò?54jÈæ?ï{á!îg? _'2Ôüb?Œ!ºô'? _'2Ôüb?￟·.Ĩ?}	aÛk»Û?€*ù?}	aÛk»Û?îÀ¿…2ü¤?†Iñœ­"Í?£ôª<€Ä?†Iñœ­"Í?ïùM5ׅ?Mfƒv?JË+×̂?Mfƒv?ìõ}uv¤¢?¼&¯tÕÈ}?¸TVpœm?¼&¯tÕÈ}?W@aM?‰¼CX=…?Žê)tß?‰¼CX=…?é"g?¡¢õ?­¼ü
@Ö?É®cyt-?­¼ü
@ÖAGN3FGL J2323.4+5849@[ïÆÁ#À3€5'À7Á»øi3À:™MüUy?þœlâ×P@
†"Gwã¼?ñ'‹h(ˆ_?ïÿeÛüëy¿Ë¢:§ñ¡¿Øh|U»ô7¿á—"¤%OTHERsnr@§mLogParabolaCas A?¶{Ogjt?µ'¾r°»c?í0–ó
?µ'¾r°»c?­ '¨«ß?¿Ñß	ª¦?î.M÷o?¿Ñß	ª¦?Ülù‰TŽ3?µn†¨YP?áɃ;U¸ç?µn†¨YP?À¶#09aS?¢݀ÐÕ?ëÒw3ñ§«?¢݀ÐÕ?Ôð#ü?ɘÄ
'?åð|‡î?ɘÄ
'?–Œ%¼…?«èçé'ã?ïO»žÉ{¬?«èçé'ã?å6‡©,3»?¶áŽð†*ö?Ւ𭧘‹?¶áŽð†*ö?¡1c ¦?=Ó߶j}?îìï	Á'†?=Ó߶j}MIXED3FGL J2323.5-0315@Sr‹`òËÀM@TƒæÀ8,ë-
$FÀ;K_Û1ê^?õðÚmÊ2ê@©8<²bé@}8ßðk¿ßû²WDy¿åÖhãªp¿äƒcþ"T—¿éN,™¢9AGNfsrq@{Q}At>–LogParabolaPKS 2320-035?ïù•…ìFB?kµ.öº"Y?I©ç|X5?kµ.öº"Y?ïÂÞô?"›ÎSêˬ?~…Æ>mm?"›ÎSêˬ?ï—&ÿK?ƒŒ{°Cäå?Š6@p™;?ƒŒ{°Cäå?ïއºž÷Ò?S¨*ûZ¦?p¼"›6'î?S¨*ûZ¦?ïô°KëCŽ?VEµÏxQ?VŸhpðã?VEµÏxQ?îòéoÖã¸?·ý‡µ? ÑiµÝ~?·ý‡µ?î^³ó½°?¢we`å›?ªÀÌüW?¢we`å›?ï¾<üÔ@?qõY'Ô<²?€pàêwç?qõY'Ô<²AGN3FGL J2323.9+4211@Z"º@Ù$À1Îÿ:cÀ8—nVõ°À;&Lké]&?Ñ32á0:@òÏ1+7?þ3'€ù9½¿âVÊÚóñ¿Û6fã}­¿Ü?_|ùa¿Õ¬HßÂÉAGNbll@¢§/\(õÃPowerLaw1ES 2321+419?ïÿ°±°‰>ú»î¤*±É?Ӕk½t>ú»î¤*±É?ïÅmnÃW?£TÛ[?}rI1@üŠ?£TÛ[?ïæK­S?gjïýkð?i´ño‰œÂ?gjïýkð?ïü"Þ ²'?$Wç
Õu?;Ùöh6ù?$Wç
Õu?ïÿ7ÕH5=?çòâÂ?YÅɀµ?çòâÂ?ã* )?¸"Ù¢Ym?¥ÖqÊÊHv?¸"Ù¢Ym?ïàWïˆÂ?xêÝg?o¨~)k?xêÝg?ïñ/Qɘ²?O"*{k3â?]¡[ñ¬A?O"*{k3âAGN3FGL J2324.7-4040@uãV¿Ê…ËÀPå}ßÿ¯xÀ8´@éÕPÀ;
®J*Æ?ë<¶ÅrÍ@
Å6ϟåä?ü*@›P©¿æ•¡%ª	¿Ó~ÉDé$¿ÕN›}ÁÄ¿Ô],bAGNbll@¯¶z—PowerLaw1ES 2322-409?ïg¼Àæ?–†ÀwI¥ ?"Èa2?–†ÀwI¥ ?ïŽÏinÀ?Ÿfš‡¸î	?ŒL9¢4´?Ÿfš‡¸î	?ï­ûPm×?'¬›GýAJ?œJ@
6?'¬›GýAJ?î¶˗v1?…y|NÍF?¤žÃCî?…y|NÍF?ïw^j]Z¾?•òýc§g?'2»3à<?•òýc§g?ëYcYÒÀ?Ç2ÜÅ­­?Қr˜´þ?Ç2ÜÅ­­?îŒâŸÍ?šFâäýuU?§?¡ß*?šFâäýuU?é<ˆÂdÀ?±dgÃ(?Ë
ÜõÂm?±dgÃ(AGN3FGL J2324.7+0801@VA©¿ìêzÀH†|à%o%À9];÷'À;*Ž:Á¿úÖMI^î£@/Ø;Ù@5æzyC¿ÄT‰ Žfœ¿æ¶à'>祿ÝQ"	ve¿àGBAGNbll@š,° ě¦PowerLawPMN J2324+0801?ïÿ,"¹º?J{A
£~?{´™pT½?J{A
£~?ïÊà'êÍ
?–N"k?.¸?zëóìô?–N"k?.¸?ïâí'y ¼?sYokso§?mn>{î?sYokso§?ïÿùsZ%÷>Ãîl×>Ê2$HK×:>Ãîl×?ïÿƒËÑû
?	H.å•v?
^9oÉ?	H.å•v?ïK狮¹*?¯™ÑaÜ+?–ƒPD°?¯™ÑaÜ+?ïÝÄ}»1?zûöU'<ã?qøC2+º?zûöU'<ã?ïÿ¶Q
^©?£<™í?k¾ñNÇ?£<™íAGN3FGL J2325.2+3957@Z`u>p~À3ûý€É¾ûÀ8ñ?Ãdn?À;^>¢‹±?øž|DŸ[@—ò'OOI?øœcÎ[˜?ÇñÃ.ñã¿àzµäå¿Þ´3ôNF	¿å¾ÄŒó$AGNbll@"T¯Ÿ¾wLogParabolaB3 2322+396?ïˆÈæä%.?½Ö%¢73.?ÍÆQEˆn?½Ö%¢73.?ï‡
Ss£?™D±F<-?Ž=k4EEÉ?™D±F<-?ë2ušÐ•?¯ÊfÞ3ç?Ã6)"½¬?¯ÊfÞ3ç?ïR˜8ùú5?uBkˆº?•¬øÝQb?uBkˆº?ïá•Z´pN?x…
ï¢|Ò?nj¥<qiµ?x…
ï¢|Ò?î(
žƒR?»›¯üå÷Ê?­Y‡fÙ?»›¯üå÷Ê?ì‹`(^ÃÛ?ªèºùm?»¤þ½	á*?ªèºùm?î›ÄO|6?'7sRÀ¿?¦C¿|À
–?'7sRÀ¿AGN3FGL J2325.3-3557?ý"YßDs¢ÀQmœýç!À8¾¨C€ˆQÀ;‹³ünñ?üÑÞú¡Ç;@­¶Ð·?þ'Ø	kä¿Ö¸§'(¿ãpPJU¿äÉHROX¿ïÿæNËaŠAGNfsrq@"¨¼w¯dLogParabolaCTS 0490?ï1‰%
Ú?¦(ðp™Z?™ÎÛcÌ)Ð?¦(ðp™Z?ïVÛ¦ÚIã?²d®3è6v?•$‹$¶Ã¡?²d®3è6v?ã+À«+gb?µšŸÕ¨&?Ù¨~©©1<?µšŸÕ¨&?îg€êm"ú?86µñ)~?©‡ñ[ºuc?86µñ)~?ís4™Ôl?¹Ã1:%?·œf\
C¡?¹Ã1:%?gç¬?³Aà?dØ?¤¦¹ƒ=
‡?³Aà?dØ?çc·‹-V?³£$Üæó?Ñ9ôé¥S?³£$Üæó?ìçîÅß·z?¨|5Ý;î?¸À‰ÏJv3?¨|5Ý;îAGN3FGL J2325.4-4758@tÿ¹ÿÖ•ÀO¡ƒ_›q
À8÷.=*,úÀ;wv¡G
¿ÂÌV|°Í@CDÁ{
@|| 9›Ø¿â®Øê,¿éêï¼TÉ¿àŠj%™í¿Þh¶ª÷eAGNbll@"H5%F
¦PowerLawPKS 2322-482?ïÿ¾zVu>û(§ê?aœ>û(§ê?ïԚïZu?ŒpC9.­?u²ˆ4ɒ?ŒpC9.­?ïâéÐ1Ü?h

L"õ?mï_è«¢?h

L"õ?ïý½ÒÖH™?Ÿ¡¢–J¥?2h#À™?Ÿ¡¢–J¥?ïÿ˜%%k?ÍΙþ?	öÄ@:Ï|?ÍΙþ?ï«Òΐê?µí:{]?
…¡xÕ?µí:{]?ï¹ù¿…LÂ?ƒqC»ËÛ|?¬Ï"?ƒqC»ËÛ|?ïñ!iËå`?P2àA£9ð?]½,éfB?P2àA£9ðAGN3FGL J2325.6+1650@Wɪàú¯ÀD®ö@c^À:02ˆéH.À;ÙÏsëŠ?ҏ‹Ž>Å@ÎÙçè\@Ï\ÿµWe¿×C[Òí*ï¿â.¼Á'ۿߊ‰|§+º¿Ü	¯j«qAGNbll@ž•y¦µPowerLawNVSS J232538+164641?ïÿ«=IÑI?›T€õÈ?0¯kñü‹?›T€õÈ?ïÒ¨D	ø°?ˆ"C'ÑÙ?v«Þñcö?ˆ"C'ÑÙ?ïêû܄е?kÏ4/,»?e#['ãs?kÏ4/,»?ïöû|7´?5Ýc€˜Þ!?Sî	\Æç?5Ýc€˜Þ!?ïÿ–ÒP*¡?ä6×3e?
KjWí*=?ä6×3e?ï6ËT ý?¯c™¡_c?™&œÓ´Y?¯c™¡_c?ïàsíZ?wàÓWg`?oíŒS>¥/?wàÓWg`?ïÇ<'' ?ht6ðm%?|a¹#é¼a?ht6ðm%AGN3FGL J2327.7+0941@VÎ]ÿú÷ƒÀGûæ Zé[À8sþk«IÅÀ;Sï«&\?êê+žQ @uiäu5@lÆ 5T¡¿ç',ÐÔªx¿çž¯rô¿/¿ìûXùé¿ÔHæ"¥AGNfsrq@~Ä@·€4PowerLawPKS 2325+093?ïÿqÌîR%?\6YÃ+,?ÆiËèÅ?\6YÃ+,?ïÎwÈA*u?ð‹¯%eù?xÄò¨•<?ð‹¯%eù?ïk…?'I٘J$?'ŽUf"?'I٘J$?ïÿH¯@?ÑþÎïøw?þÿeÛA?ÑþÎïøw?ïýÆ	ª?3{F
—þ?1ϲóªê.?3{F
—þ?ï>/Dz?°3\Ú¾«a?˜>z$Žs®?°3\Ú¾«a?ï/··«—7?"C±Ö]aˆ?š		Dç#?"C±Ö]aˆ?ïýãWu)D?.‰·kƒv{?0åBqÓg?.‰·kƒv{AGN3FGL J2328.4-4034@u×TߋrÀQJërªÀ8r2$?ziÀ;M=5´Ã?ï¹+è'#~@Ïz>üë@wö?ŒÝɿݵÓ€ná¿çñ@/׿ã¥'¹ßü¿ç{$Ö³šAGNbcu@‹þÐHðPowerLawPKS 2325-408?ïÿ'ãäZL?U5€xð?G'"+´?U5€xð?ïËXÉ4?—;׶NŸå?zr}PÛ¶/?—;׶NŸå?ï«è-GÙ*?ƒMBƒÖ4e?…ô£ºá'?ƒMBƒÖ4e?ïú?$
ÔÎ?1j¸wz?GnѽmD?1j¸wz?ïÿtòÆ0¦?ˆbÆQ¡ý?a®Ò¤¨?ˆbÆQ¡ý?ï-EÝÒ%?²~Þ±'Š?šWDJâÆA?²~Þ±'Š?ïQ®‡*N??ê·Õ€?•Ê?B D??ê·Õ€?ïó§©@ši?M‰½*-Ö?X°­÷½mâ?M‰½*-ÖAGN3FGL J2329.2+3754@Zb'!%¶À6*ÅÑqwÀ9^'åp1ÁÀ;rùÒ¿U¿±Ž7°ñO
@Êt[òo?þÖϟåãõ¿ÚY^ÅLÄ¿æèϼý]¿ÓœÎùÁ¢¿ÉËV=ô?AGNbll@¨IA [ÀPowerLawNVSS J232914+375414?ïÿTX-$?ÅÕ<!ĕ?•|T¸¬æ?ÅÕ<!ĕ?ïÑ]³?ߋ®	?wQx袤?ߋ®	?ïé"aù?ZºƒØ¿Ú®?fݞš¢¯?ZºƒØ¿Ú®?ïüبÎö?#Ý]ÊbUB?9:¸R\?#Ý]ÊbUB?ïý̈üŠÍ?3ÁN4PÂÆ?1›¶ŠW:±?3ÁN4PÂÆ?ïÇ9 CS?±kGíB?çÚ?Ç®?±kGíB?ïÕz\O?wœÎç'?uBÑبx?wœÎç'?ïíãÐ
c?WCùH
²\?bäû¸p?WCùH
²\AGN3FGL J2329.3-4955@tÀ@%NÀO(?ßéàÀ6¢áÌ8RWÀ:Ë%Ü2›@Ñ´d ;	@ ft"§lk@…ž†"W‹¿à®•ó­óT¿äâSþô¿æ|ÖJ­€à¿ê(…	¿œAGNfsrq@w†Â&€LogParabolaPKS 2326-502?ïÖÀQ>a?wä)ÿè‹û?töÂÃ'•?wä)ÿè‹û?ïÊéxÃÐ?–ˆÏdªð?zÿ‹VÛçñ?–ˆÏdªð?늦¹+Ÿ?¬žN)ñ¥{?ÁÕeQƒð?¬žN)ñ¥{?ïýEeÑÅ?,ß(‡€Êu?5ÔÒN¯½?,ß(‡€Êu?ïU/7Xº_?•PŽ³˜‰?•ZÇì?•PŽ³˜‰?ï0¢Bµ‡?²ëgÄ>Ç?™ü«²å ?²ëgÄ>Ç?ëБu]Ð?ªÞÕóH)?À½º*ˆ¿­?ªÞÕóH)?ïþèæ©?(x?±ˆ?&!~uM†ñ?(x?±ˆAGN3FGL J2329.9-4734@t÷:ÿ°NèÀP_¿î—ùÀ:*Jmâ\À;½êi•ÅÐÀq—:ï•$@Á3¼p@Úf€'ŒŠ¿ãýß-;f¿Ü•AþÓ¿è÷%L¯tç¿Ë™ˆ/lˆAGNfsrq@Ÿ6Ü(õPowerLawPKS 2326-477?ïù0×–Õ?]™	(*4?K=ˆˆç{?]™	(*4?ïÕvíM"?‹âLHª?uD‰Rìºh?‹âLHª?P•o?…©‰g!–6?ŽÖ+Ú¤Q?…©‰g!–6?ïÿþa‰ ¿>¦ŠÈŸH>©êë"B>¦ŠÈŸH?ïó½Y'B?\^*»¿?X…LW‰æ1?\^*»¿?ïq"+èÞs?§´N·Ú3?'Íz‰Ãi ?§´N·Ú3?ïi×µ5?—EnùÎ\?ŸÒÅÇ]?—EnùÎ\?ïÿÌ`b¸©?^^FµÓÑ>ùÏÝ'#—ë?^^FµÓÑAGN3FGL J2330.4-3726@vJÓß°Õ ÀQ"ÓÀíÀ:TX¸þ¹¯À;öBzÎÓ7¿à²$'( @*éÓmо@Ž€¢§µ¿ã/Bóçæ¿ã8ßi nÏ¿æȹz¿áÁÁ¯@—AGNbll@"0féxÔþPowerLawPKS 2327-376?ïÿ.vØF? '¤Tœ†&?º6(Ø? '¤Tœ†&?ï×OBf	¨?"[•UÓÎI?tX^çÈò?"[•UÓÎI?ïª&ô?z³tA‰wä?…`65A€?z³tA‰wä?ïüœü$©-?'ô!˜¤+?;ÿ¹i¼?'ô!˜¤+?ïüÖ{ˆr¼?="Ó+Ù?9L"™¢Á?="Ó+Ù?ï5Çÿw]É?¬¥ñ¸0áß?™G
5à?¬¥ñ¸0áß?îï'†'çà?˜¤ƒÏÐ?¡
‡šAý?˜¤ƒÏÐ?ïÅ+äñlû?r}¡A1çA?}j
xÎD?r}¡A1çAAGN3FGL J2330.5+1104@WD¶ŸÏ=ÀÀG†"`LpòÀ9¦5\_VÀ;‹võ)ã(?ÅÚ­Âè¿¿@|û£$ð@p¯Àw~è¿æV< Õ^¿çüŠ I¿é	¶™üã7¿àpý~ÎðœAGNfsrq@‡½í(ŒçPowerLaw4C +10.73?ïÿ.«±k•?TqH|‹?*†Ê¼¨è?TqH|‹?ïÁmU1Ï?"1|éyoœ?9IR§hI?"1|éyoœ?ïÛÖf|-?l"°Ëtž?r÷Gòud?l"°Ëtž?ïìwBèÄ
?K	g/ÆþÛ?cˆ½:÷åb?K	g/ÆþÛ?ïý
†È¨ó?95³[G?7"ÉtZù?95³[G?ïõŸm²Ð?±ä=ø?Ljn?±ä=ø?ï£o`,‡ë?ƒ|º×%?‡$'øM¡L?ƒ|º×%?ï-bÖ[?Šºßì7–Ý?š_¥4"?Šºßì7–ÝAGN3FGL J2330.8-2144@FtqŸÀQº ÒH7À8é¦W>À;'<b†ÝÕ?õ" pãÂÞ@±±Bؗ±@(‰‰V*"¿á‹³¾¥¿æ]'O7¿æ,‡JÀ J¿íÔo6"nAGNfsrq@{t¦Þüz:LogParabolaPMN J2331-2148?ïÞªýM?hVê~?pÿ+
oŸ?hVê~?ïÊ°ºmá?"gɤ	›E?z§¢þh—k?"gɤ	›E?X){"?•Ì×ò`ST?¦¤*yøªÑ?•Ì×ò`ST?ïÜz¨£ÞÓ?W-&†«ðÿ?q«žBb‰?W-&†«ðÿ?ïÜiãH;?oÛû4Zwà?qËyE_?oÛû4Zwà?ïS¤ª™Ç?£™û«fÞw?•‹j°6¹Ü?£™û«fÞw?î聄W›¦?––Øñ‰ŸÅ?¡wç»b, ?––Øñ‰ŸÅ?ïºf…ððC?ssdâ¾â»?f^ŽÂ¯I?ssdâ¾â»AGN3FGL J2334.1+0732@VôªŸæºµÀIM]߯' À9P>±·!À;œ‰çÒ¿¿K\¹ƒ2¿@*^%$QÄ@	À¿£C'¿å"«ÂªÎº¿èRk);/¿ëŠwV	L¿°qÀ•9–,AGNfsrq@ƒ8ð£×
=PowerLawTXS 2331+073?ïþŽ*GÃ?2…Ò-Õ3š?']öË?2…Ò-Õ3š?ïÆk²‰2L?—õ,Î{^×?|Ê&Ú69?—õ,Î{^×?ïÖPpI­ã?mþÕq'Âq?t×ÇâF–?mþÕq'Âq?ïþ5C?,?›âPÙ?,«Î>Š†¶?›âPÙ?ïû èBt?D
—	¡Ï?A|_)P2Å?D
—	¡Ï?ïv´´Ÿ|?³KøSž?±)il†?³KøSž?ï£mQ€êæ?"GŽ¦Ï¹?‡$«¦¤~?"GŽ¦Ï¹?ïè;Uõ²?c㼩SÂ?gĪ6â?c㼩SÂAGN3FGL J2334.8+1432@X$՟Ú%{ÀF0•ÿ±%§À8èºÅcLÀ;<
MzÝ?ó
…örc@CÒÏÆ&j?þ
j¬¾d?äh—ë»ò¬¿Üƒm
¢ùÈ¿Û»ì,
þ¿àÈT˜ÉAGNbll@¡áóZ…‡"PowerLawNVSS J233453+143214?ïÿXžˆ†?N:é'¾?þÆ bÁ?N:é'¾?︄ú-á˜?]_J¡?ÞÁ}Ÿä?]_J¡?ïžò ÄEÀ?ƒþUø±_e?ˆCwÙ=d?ƒþUø±_e?ﳝz¾{ë?`âñ^ö?ƒ¡`ß%+?`âñ^ö?ïÿAzYôy?Zñ¶‡¯ú?к̬m
?Zñ¶‡¯ú?îù[<«pË?´LVH¸µÑ? jL8¸E?´LVH¸µÑ?ïi;ΕØM?'˜>ºJË?'؆-Dön?'˜>ºJË?ïdSž…4?}[Ôa "Å?"uŒ1Çn?}[Ôa "ÅAGN3FGL J2335.1-0133@U
>?Ö¯¥ÀMGy`>.9À9çÜÓ«
_À;–a(	4?äÔºŠˆ@)\šµ£@°Jߢ<€¿á|8xóÌ¿çlmiÃp¶¿åd*eÈö¿îáõrª¹ÊAGNfsrq@³°ò{²ÿPowerLawPKS 2332-017?ïùÝ®"É?E+ÄÀ	KK?H‰FE×}ò?E+ÄÀ	KK?ï¶c45oV?–,œ[¹æË?'g2í|À|?–,œ[¹æË?ïœLŽêÓ?
Óى†?ˆì܂dƒ>?
Óى†?ïR4wÖ°?sB®ÇBe&?•¹qåò?sB®ÇBe&?ïø8u?Tr.î(,?O³õ¿?Tr.î(,?îJUþSu?´Ë
‡/?«Z ÎH´?´Ë
‡/?ï+
DÒlõ?–V7/œCÑ?šž·jÙË_?–V7/œCÑ?ëé.
É0$?¢c÷肫"?À[GÈÛ?p?¢c÷肫"AGN3FGL J2336.5+2356@Ym¢£Y6ÀAê.Íû¡À:SefŒ&À;àø‰éù-¿Ôl£÷ì`;@
"yöf#K@ã_`bÁ¿éD~Lêœõ¿ãKä;m-D¿Ü4H‰()·¿Ô/X×*ÁAGNbcu@¡(Ð|"µÝPowerLawB2 2334+23?ïaŠ^"3?¼³ò$9	%?Œ§kÊÏ(?¼³ò$9	%?ï˕ë—ƹ?'Ž6±È?z5
4̏_?'Ž6±È?ï×ké!"?€0ï—k+É?tJQ@ß?€0ï—k+É?ïü¬?}]=?%Åi?*€'?:ž)Rl?%Åi?*€'?ïþbü¤€Ó?1D}
{‰
?)Ð7$ü|G?1D}
{‰
?ï0!öŸÙû?±¥™%W1Ó?™ûÁ*Lò±?±¥™%W1Ó?ïȖL»£?'UÙ¯íñ›?{´ÙÀk	¢?'UÙ¯íñ›?ïݲçã?daît–ã?q&‹þ¦¶?daît–ãAGN3FGL J2336.5-7620@sIÈ MÀCú‹ Z›À9Ü-$%y6À;ΞÚK:'ÀßU®dÎ@é¥J§Ä@¤2`Ov
¿áre¼â
¿åÕï°Hÿñ¿å
1÷Ž¿Ú‰N³A`sAGNbcu@{é^ž	PowerLawPMN J2336-7620?ïûß.¤-F?BÔðŠæ5Ù?@ƒEo<Ð?BÔðŠæ5Ù?ïÚ§LÏUW?‡Îgã]?r¬YƒÀ–?‡Îgã]?ï¾µm"4?yC€êÐ?€R¤Š´ß{?yC€êÐ?ïÿý§Ç@>²Í'~
$Æ>²ÃKµôÄ>²Í'~
$Æ?ïëägüœ&?p9œZžo?d—Æêºe?p9œZžo?ïE±.Ðg?°ãŒÊÜ»5?—G©Ý•!?°ãŒÊÜ»5?ï£È,æ?•{ìɾ7?œ>Œ!Í4?•{ìɾ7?ïÿq6ñP?zO/h;?£§±&5?zO/h;AGN3FGL J2336.5-4116@u˜`@|ÇÒÀQG8à^*À95±/¸TpÀ;¬r9€
?óÙ—ïun@Ô÷!'@ê?Ðz¿Ü…¹}(¿á0ýg¹œ¿égÄ^á"6¿ä©ÀkžVAGNfsrq@²-VPowerLawPKS 2333-415?ïüôw¶šÜ?A)2
ö,?8\B™9×_?A)2
ö,?ïÏ;å¼æX?'××ùÃÔ??xb
#œ—Ç?'××ùÃÔ??ïV"eIu?";zxJ?•;º6	a?";zxJ?ïí…uLn?L'™húÎ?bzà™ÑÙl?L'™húÎ?ïù§ ?Pôí¤Qe?Iû¤ÌëlÞ?Pôí¤Qe?ï$ÀÜ P?°sèjn%%?›gäxŒš?°sèjn%%?îj)Qæ…8?žÄñ™V?©]jß÷?žÄñ™V?ïÈOhY@õ?r"5ëÞÜ?{ØKÇ°Ù~?r"5ëÞÜAGN3FGL J2338.1-0229@Uï¤hÀMâ'àÙìÀ8µçïhHÀ;n\Âxµô?à¥ß‰N.@sôI"qâ@÷®XëT¿ãæ!¦² •¿æÙ{ªD¿é"~‡øB¿äíëÅ­ÁAGNfsrq@"[^½çPowerLawPKS 2335-027?ïÿ¯þé]/?Îâ±vI˜?Vuþc.?Îâ±vI˜?ïÂYœ(• ?'°jƒõ"?~Ó1íÅ47?'°jƒõ"?ïÝ}CDØ?]É­%ò?qA^>V¬O?]É­%ò?ïôù3)š{?=\ß¼¶Úp?V
™ñƒ:ˆ?=\ß¼¶Úp?ïþùҋÊñ?%(÷? bٌA›:?%(÷?ï+O	?±ñ _Q6c?š–àîxá?±ñ _Q6c?ï¬{ƒ®ö£?¬Œ¸M?"á!4?¬Œ¸M?ïÄø§"y¼?p	G@³?}ƒ¬OQµ?p	G@³AGN3FGL J2338.7-7401@sYPà"'ÀE%àdYFÀ9ʝ}SèµÀ;¦¶Iӈ©À@2¯´ì@Mlr¹±?þ4¢ÿžÜ$¿åÛá"ÒVò¿ãkܬ¿â¿Ê[ý!(n´¿ß˜Ëe;˜AGNbcu@¦;šPowerLaw1RXS J233919.8-740439?ïÿvH‹p?ê¿Òö??ôî2 D?ê¿Òö?ïÚÝ}@•?"²¢H!©?rÀB¿Š?"²¢H!©?ïðQŠóJ?hš^ÖD-Î?_Ã\Öۜ†?hš^ÖD-Î?ð=ϟÖ	2
= –p…SFa=ϟÖ5íí±?ïÿ'•L
£?[Š€âô?Z¥u<±ê?[Š€âô?ïN&ÉÃX?«"Yk?–;&ǔÿ?«"Yk?ïòRÝûý?lku-üU?[óZ"¾ö
?lku-üU?ð>f@Ôµ=î{¯éÖÛ¹>f>ï®ØAGN3FGL J2339.0+2122@YPyámmÂÀC5ëß·‹À9ãIŠÀ;Àaâs'¿œô
Oûp@ρó_³š@nԀu¿ååª	ºz ¿âÑOS'ç"¿áАDõí¿ØswšÚûþAGNbll@˜¬@4mÅÖPowerLawRX J2338.8+2124?ïþ"?§#µ?+;î­B$?&ÌCê7,?+;î­B$?ïÂÂÎ#íy?"¿ÐPj?~ž˜Í¼ïß?"¿ÐPj?ïãD«U®³?^ëAº\?l»TÌ­dŸ?^ëAº\?ïèzð·Ç?R¡ì¹N-F?g…onؽ?R¡ì¹N-F?ïüa,Î?B Ö-"	Š?<÷î"ÂÍ?B Ö-"	Š?ï+$¼«u?¬Óù/äñ?š›heió+?¬Óù/äñ?ïÀ	yÀº?€0ÂýU€?ûCk[@?€0ÂýU€?îÝü"f>?"~\ˆ^aI?¢ ?t5ç+?"~\ˆ^aIAGN3FGL J2339.6-0533@TUGÀ'áÀO<OøÃÌÀ8:[Ê+1ÝÀ;MQN§-@M¹2;;•@
‡ûÐñI¯@=I#àYò¿Øú"¯-¿ÖßóÙ^´¿áÇívÝÏK¿ìm¯nJ¾ôPSRPSR@òà`þG™PLExpCutoffPSR J2339-0533?R'MÁE,t?Yö狓"@?ïö¶ÙN?Yö狓"@?ÁV=A‡'d?Îðٕ÷½U?ëªp¯žg?Îðٕ÷½U?¼GÅ!ÃÛH?©]¦§³³'?ìw[DŽ—?©]¦§³³'?¶ÛÎç<?vÎKqªQ¢?ï$¶¤ ?vÎKqªQ¢?l«R+­?iõÓºPk!?ïãTå¤Mì?iõÓºPk!?´3&	ÌSø?Ȁ…šøÙ	?íy›?-±?Ȁ…šøÙ	?µ¬€0¡d?±t˜ïÉ?íJ|PªC?±t˜ïÉ?b¶@~?Wâ|¥?ïí~êQÿ?Wâ|¥PSR3FGL J2340.7+8016@]öaՈ@1Ó8€z
ãÀ8Kê¸pvÀ;$'ÅA¾?ìhSbÊòÏ@Q\ÿ_q*?þ¦½žÜy"¿É
BÖ
Û¿àŸ@ŸNÜ©¿Ù-ûȇ»¿àPºAGNbll@ xÔýó¶PowerLaw1RXS J234051.4+801513?ïãøªmž¶?d
`›ì8?lUã)»?d
`›ì8?îíK!Äÿ?¡ähû»#Œ?¡'ëJt?¡ähû»#Œ?ï•
ôÙ8ô?"Àm¾«i(?Š½BÔ–Õ?"Àm¾«i(?ílh'—u?"‰D­q!\?·4œ¹»vY?"‰D­q!\?ïµ?¬NŽ?|eÎ(Ö¼?'¿°
µ.z?|eÎ(Ö¼?褏œÉ,?Ç'×ß$"?ÍmÁŒÛMÍ?Ç'×ß$"?îºÏÓ×?›b^\S?¤^SVC=?›b^\S?ã:¾†§¾?¸±ZYiˆ?ÙՊ'ò°"?¸±ZYiˆAGN3FGL J2343.6+1551@YŸ'xÀEü_ !¸À:@µ¥8À;Ô+ç—r?éÿ»ä¬@´êÓ@Q¥ÿÙi"¿ä¶›Þuõ-¿ìårÐ×ôH¿àKcEŸœh¿åm{ 1ίAGNfsrq@€J ù	kºPowerLawMG1 J234342+1542?ïÿ'üéÂs?œIZ*ï?@ÆÆ£?œIZ*ï?﬩…I&?-8àUÈ?"Õž·Î~w?-8àUÈ?ïÍí8¡Î?}Y?»]¸?y	d|Ñ?}Y?»]¸?ïK…ŠV?wì¶"?–N¹ŒÙ6?wì¶"?ïÿ–«w?U2^v
x?
U-Э+ó?U2^v
x?íâöÚ½P?¼Ï.¦Üx;?³xèKOÖú?¼Ï.¦Üx;?ït^¨µt?Ž¶ìÒn?'lT1ȉx?Ž¶ìÒn?ì`ÎHÅ8%?¤Y	¡2wô?¼ù¹Ö>Õ?¤Y	¡2wôAGN3FGL J2343.7+3437@ZÝþD5À:2Þ@'—GÀ:Iá`ÈWÀ;¼—•³[¿Öà"·Â@"†w}åß?üþ –
¿ïÿñ;äT?ïþ ûh%¿Ìi•Zo¸¿Ò·½áÍdøAGNbll@µM`A‰7LPowerLaw1RXS J234332.5+343957?ïÿoÏú1h?erDËô?	
ë3â?erDËô?ïÿO‹®t?tI&_?~ XF‡]¶?tI&_?ïè+€"îm?dùNKĤâ?gÔ¤Ëø?dùNKĤâ?ïúÄ<"
?1/íJ€v?DïۏvÔ?1/íJ€v?ïþéoù?Ð?"C†5€-?!iï
0ö?"C†5€-?ï;S]þ–|?¬¥´:FÝ;?˜•"Ghu?¬¥´:FÝ;?ïäP€1Né?rõÊé9^?k¯µóçv?rõÊé9^?ïé>i?]zÙ=à£?fðÁ¶P®ù?]zÙ=à£AGN3FGL J2344.4+0549@W'?ïXÀJ¢‹ Z›À:5¾ aŸÀ;·"ÌÐþ‹?âqš¾ÿüò@"ÕÁ=!Ÿ@‹‹À"§¿ã3Ál;¿®f@q<â¿âÿñÊ)¦º¿ïôV©"ôAGNbcu@™‡ÊÀƒoPowerLaw1RXS J234354.4+054713?ï+×IR"\?–à1Üۈˆ?š…Ò?Ø|?–à1Üۈˆ?î)á¬Ç?±_÷ºË¾?­aå0‹<?±_÷ºË¾?ëU•	Î?«È
ÜrÃR?©¿½«ØÈ?«È
ÜrÃR?ëm;î©Òˆ? ¥µy҇?ÂKEXµà? ¥µy҇?î¼ó¿'<?¢«‡$Þ?¤0ħ@?¢«‡$Þ?åòεôÝÒ?Î(ZiOqO?Ôb"D\?Î(ZiOqO?éÂV²qàK?²ÜèãÁ¡o?Èö¥68~Õ?²ÜèãÁ¡o?ØDèâ×ü?·p—cØB?ã݋Ž"?·p—cØBMIXED3FGL J2345.2-1554@Plžà*w£ÀQ¿_ã•fÀ7>/GìÀ:ŽÞ¢¸&?ýdþ¿¹@ü½å©<¥?þ¹Rý(	^¿Ü±—¾ß5¿âFA¹¾J¿áº™ˆ@›¿æ¾ä½ëoAGNFSRQ@‰ÎPHðLogParabolaPMN J2345-1555?ïýÆÊ?¦?2¦øú"Ô?1ɬ»n-k?2¦øú"Ô?ïÄ\$\ð`?–'¬kgj?}Ñí̸\(?–'¬kgj?íCâ'ì"?¥»V'9Ò)?·ýàí2v^?¥»V'9Ò)?ïÿb'šé??×Îå…dî?¯©§{?×Îå…dî?ïô1÷Z%L?Y‡0?˸t?Wœw°hy?Y‡0?˸t?ïf¸€[ýN?¡ÆùB.uJ?"(ïö8$5?¡ÆùB.uJ?îsC׸? Oˆj§{ ?¨Î{Ð:R}? Oˆj§{ ?ïÿÃxK|f>þ-ÑWÛl>þCÕ®)8>þ-ÑWÛlAGN3FGL J2346.7+0705@Xß֔ÍÀJ/&à>™™À9*NRsj[À;1dÂ!x ¿ðò㯽Gt@ì±Ííß?üu§ALü]?ï]cdÿ¿ææ»"!àG¿Á÷=ëTÚ¿ØKÈ·AGNbcu@¯óÞšPowerLawTXS 2344+068?ïþ®Ãf5ƒ? ‰©,KÇÛ?%ȔÅӖ? ‰©,KÇÛ?ïϟËm?^èÿĂ?x0v-¤?^èÿĂ?ï®ú¾?ÚÔ&OK?~¨'¡J´ú?ÚÔ&OK?ïÿÕJŸ¶i>ëqnBd>õZÎtµ2>ëqnBd?ïþ¨àg?%†fQûR\?%qýÓÙ3Ž?%†fQûR\?ïRtø-+e?ªì
eá^¿?•±`ó{[m?ªì
eá^¿?ïÂ5a-8ë?'ä&»—¤"?~åOL†ÒÖ?'ä&»—¤"?ïÿ,ʨ1?ùq•&?fª
Up?ùq•&AGN3FGL J2347.0+5142@\8åÏxyÀ#Îã¿ØrÀ87¢ò(§À:éß÷KüX¿ñîéµ:ßÐ@u'Ý7©?ü…2ªÍ¿ØGÏQâJã¿Ù	žkÝÁ¿ÝëØM*øt¿×|ÞÀó®AAGNbll@§iÇ»/ìWPowerLaw1ES 2344+514?ïÿ–˜Þ2Ñ?–£Ÿùï?
YÖÐñRš?–£Ÿùï?ïÆY_å[?‰'Ìu$t?|ÓOúên€?‰'Ìu$t?ïÙvc!Û?w쬞×?sDÎeÒ
…?w쬞×?ïÿì$çý>ݲƄ&|å>ãÛï¼?b>ݲƄ&|å?ïþ'¼TÑá?'oì\Pɽ?'Ô9‡ÐÁ?'oì\Pɽ?îÝP¼W?¯AP%‰á?¢/
ñªå?¯AP%‰á?ïØÒx¢?"6Œ,ÁN?s–Ówo?"6Œ,ÁN?ïÿQÅM/;?Ĺ£!³?ÇS¤öÀÇ?Ĺ£!³AGN3FGL J2347.9+5436@\ož²gÇÀ"•¿ðExÀ:…gÖ¨î¡À;³0¨LÀ
­óõ"@ÏTБÓR?û»ê^Øþ^?ïÇôЙWw¿Ø$ë"/š¿éqF_®¿°ÿçÆ5¡AGNbcu@Ä$VPowerLawNVSS J234753+543627?ïøÅ
2:?Qjéòy†?LëÊòìsÉ?Qjéòy†?ïÏçâv`?ƒº®(G?x?/Áâ?ƒº®(G?ïo6•´?"M««©4l?'<Fj8&?"M««©4l?ïÿÿû´}>W¯epë>B$՘çm>W¯epë?ïÒ~}"N?xò^)žn?vÀÁ™B|Á?xò^)žn?îèPV¸&*?°Õ^S¸Þ?¡zú"¡¶]?°Õ^S¸Þ?îM[ä"y*? :µˆ'µ?«*A¸€;Y? :µˆ'µ?ïÿþÇÁ~>½pmð…Z²>¦ñ#+5J¹>½pmð…Z²AGN3FGL J2348.0-1630@Pe ÕúÀQøM@$³>À8@¨E.À;ýFèÞ?éûß+k‹@g
[@ŸmŠNοÖò"†ì)¿åG@ÿÞ*}рÕl¿æ—ÊšvAGNfsrq@"ô_ö"PowerLawPKS 2345-16?ïÿ¬á¨"¢?J'ÙkÊ?ǚäÔ»à?J'ÙkÊ?ïԕ]l91?‡߀Zbµ?uµQiχ?‡߀Zbµ?ïÖPœÙÅ?v²âµÖ1ï?t×±…€?v²âµÖ1ï?ïýmª*??=o"ì?4'°FÔzä?=o"ì?ïÿµFÀ¦?C¦§Ì?®MOóê?C¦§Ì?ïL@ÿéH?¥y¶ú"|?–wßÿgP]?¥y¶ú"|?ï±2?†õ€¯™´g?ƒ» 4xa¡?†õ€¯™´g?ïü7ÝM3Ì?4Ec.°¢?>AõÚJp?4Ec.°¢AGN3FGL J2348.4-5100@tTŒ_¿ƒ8ÀO¦¿Â"OÀ:AÖ²ÿœ-À;ôäq.A?æxނE®Ð@|+Nbc¢@r?³Ê¿â˜ .wüU¿àØÉEiþ¿è&•GœÄ¿ïÿYsÜ1AGNbcu@s½p£×
PowerLawSUMSS J234852-510311?ïj6"ÿ•'?"eK*Ã'?'¹-|±í?"eK*Ã'?ïŽ#c~ÌÜ?—Öè¡Âò~?Œw'ýõ?—Öè¡Âò~?í¼pȃ֩?ŸÎgwç^?²y¼½1»?ŸÎgwç^?îDn€"?Ž±->d…4?®»¹óäæ?Ž±->d…4?îolà[¨{?©[ƒÇ:à¨?©	1õùõX?©[ƒÇ:à¨?êÚc:·â?Æ_=ÕE
É?ėÎs y?Æ_=ÕE
É?ꘇâѵ¯?²$Ê`#[?ŝàt¹)F?²$Ê`#[?ãstZ´›?¸Ld
™ç4?ÙÿJ–É?¸Ld
™ç4AGN3FGL J2350.4-3004@0ð›_lw"ÀS-ŸàÛxÀ9åÀ]RÁnÀ;ÂáåbÅÈ¿ìR@ƒl @ûÓ
ÔoX@¤ã@Ì¿çK˜³{Ô¿Ú·Éφ)i¿åÀ«°ÍÌ¿ÔÃUqÃß
AGNbll@ ¡áä÷eþPowerLawNVSS J235034-300603?ïþÑê÷bÖ?U½A)™?"áQT"ã?U½A)™?ïÖù´¤ž?ˆÖ¯?A`'?tƒ8'
ˆó?ˆÖ¯?A`'?ïÁRÔôç?{íª"ÏF?V–ÓÀ,?{íª"ÏF?ïÿϖß2´>ëÚ*š©"~>ø4ŽÍó­>ëÚ*š©"~?ïý·)2ºy?1ޒgíø
?2F¸sW^§?1ޒgíø
?ï‡ÕÃ&Áò? ·ö'õ;?Ž
@žWy? ·ö'õ;?ï^Ù/9\ ?‡º"t?"$ÚÔ|?‡º"t?ïý¦6¾‹Ÿ?0ûì‹ÇÄ?2ÎK†÷å"?0ûì‹ÇÄAGN3FGL J2352.0+1752@Y⮁ˆ*ÜÀE_H *AóÀ9èéuyÿ À;½ŽK‡½Ï?ÕUÌËJ@Á@ —ºœH¡@ô_¸Í<¿ë
õ‰Y…'¿³íÁ±]'¿Ý:O®áK׿çóijMËAGNbll@¡-'hr°PowerLawCLASS J2352+1749?ïÿ?òo"Ù?*"º…?²«éé?*"º…?ïÑÝi–áG?"ꜷr‰?wK6Ÿ Z?"ꜷr‰?ïì
<S˜X?Y¼"Å°?còÃÍcçV?Y¼"Å°?ᅬÖÖ?`àvÎĘÔ?€?¹Zªr'?`àvÎĘÔ?ïüCC»Zx?>*‰éØx?=åà䋈?>*‰éØx?ï\ýå|?«L2¬Ù?œnTaûy?«L2¬Ù?ïÏ憗Ý?~ƽã~¬?x½É$?~ƽã~¬?î\½â'ö?'U5c$—®?ª4!ÙdLë?'U5c$—®AGN3FGL J2353.3-4805@tw7À*ýÛÀP‹Ã¿ÝÑÀ:¯pÂ	û,À<
K³\¹?êgZ v±Ò@
ÕÇèa}É@x x™¿ì#ÞùÂq?ÝV'®àõñ¿Øhæ62õ~¿åÃ{GýxAGNbcu@¢Þ€A‰7LPowerLawSUMSS J235310-480558?ïêúø^?oôõKKKç?er§núK?oôõKKKç?ìÊ%͑e:?À,üÝ?¹®Ñ"tÖ0?À,üÝ?ïdúb~œµ?Ž)«rº&?"`³¸ÃoE?Ž)«rº&?ê®s¢ÜZ×?¤\h]~º?ÅF1tŽ"¥?¤\h]~º?ïØJ¨3ª?}ÑÞ_im'?sñÚ´Õ&é?}ÑÞ_im'?àT'¥?Òöß3ÆoÕ?ÞßWÙ°µë?Òöß3ÆoÕ?îÈ\½<®T?™ùý6Àê?£z4,5È?™ùý6Àê?Ù|Ö CÓ{?º'P½1Ï0?ãA"ïÞC?º'P½1Ï0MIXED3FGL J2353.6-3037@,*"øÀS8[ÿÛÀ9öøŠ/À;½Ÿ_¬8À
ågù8'@=L|ÛGå@Bm€ac?îþ>Ôüò¿åŽ-'*'N¿á4òX«¿ë@–®Ù¿AGNbll@—°õ\)PowerLawPKS 2351-309?ï÷"u½hÎ?Q"+ØÿÁ?P÷yô_?Q"+ØÿÁ?ïÙO‹"¯?Œ¼ÃFx"?s|ØTR°,?Œ¼ÃFx"?îÇòᚠf?—çï4A?£€Ñäž+£?—çï4A?ïÿûR+,>Âñ"œdÄC>Ãó&r"Öw>Âñ"œdÄC?ïöŒµõ3¸?YÚGƒÕ®?Ræ"ÿ›?YÚGƒÕ®?ïw¤†?¡%œ-þž?'o3Z™?¡%œ-þž?î¢7ø¿Å?ŸUçÞ¹ë?®UÜ~¼5µ?ŸUçÞ¹ë?ïÿ¯Ò}?
Œ~î?š‰´¹¼?
Œ~îAGN3FGL J2353.7-3911@u'ÒÀa"ÀR>"ßöu=À:š—Ëc@AÀ<Õ,ß@¿î¹Ò@Ö@ƒÊ${à@?[?kд¿çxS¨'Ï¿ÛQ´}¡¿à'-Èä׿ïÿZãÁAGNbcu@'|Õ*™1PowerLawNVSS J235342-391442?î‡R<7é¦?°jÊàI½?§ŠÜ=]Lš?°jÊàI½?ïÌ
» ˆ?'7G?yù"UìKè?'7G?멵¡ôP?ªmÇ:³ýj?ÁY)x/¢Á?ªmÇ:³ýj?ïü©õÃwJ?.Š~QÉ
?:°S"üµÖ?.Š~QÉ
?íi"h=?½/ÒÒ0 ?´¶ìÀÑú†?½/ÒÒ0 ?ï0•Ó;|?¯`ƒŒ1¿$?™üÍGP^ƒ?¯`ƒŒ1¿$?é.Ë.‰w°?·_5gË?ËDÓEÚ!A?·_5gË?ïÅâ Â3?u¢n1½c?}¯ú
â"?u¢n1½cAGN3FGL J2354.1+4605@\+'ÿÀ/EšÀá@À9øÈHٍ¥À;Ñ*èáÖI?êÏ	\8ÿÀ@‡Á‰LÅV@Õ?qZ
¿ÞÆüE¥¿ä%~‹•¿îíi­÷'¿ïÿŒ"ÅÁ¸AGNfsrq@"XÈK]ÌdPowerLaw4C +45.51?ï&æ¯Þ? ¤ê-Û°?œû#(Lp? ¤ê-Û°?ëñQHI?½€"ØAu?À:»ÎÞÛÿ?½€"ØAu?íÕÄ¿Pý?›ŽBWa'?±QÚÁò?›ŽBWa'?éÉðàŽ‡?ŸUcËÁC?ÉÈØ<}Åå?ŸUcËÁC?é•~Ý*½ï?ÆùKˆ9?ɪ‹UE?ÆùKˆ9?ÚoR{Öm¾?ÑV—x¤xè?âÈVÂÉ!?ÑV—x¤xè?åӘÆxó?À‰ÄFbÝ<?ÔXÎsý?À‰ÄFbÝ<?ÉÅ|mÜð?§‹UßtØ?鎠äˆø"?§‹UßtØMIXED3FGL J2355.5+8154@^7†6`å@3@à†7½À9撚Ϡ½À;ÊÛø¹º¡?Ú}'õ2@
áö#l@óðX•m¿épҌÄù¿çä{Óh¥ä¿èëh0"•¿éÃ剠ìäAGNfsrq@tY÷eýŠÛPowerLawS5 2353+81?ïõÄëàkï?UãËÚ¢æ?Tv(ÀYr?UãËÚ¢æ?ï{¬ðIºÅ?˜™j…ëøó?ŠaöȧW?˜™j…ëøó?ï'T
e¬?"KÑI:.ñ?«%ï?"KÑI:.ñ?î`Æñ/qv?†á¼^oÀæ?©óì-™?†á¼^oÀæ?ïÀëóâ?"ÿ"£ªLl?Šø÷?"ÿ"£ªLl?é7û\µÁ ?ÈU"­e9§?Ë (û?ÈU"­e9§?îa±$>'|?Ÿ¿$4ì?©äí¿†t@?Ÿ¿$4ì?àðQ9«?·å[Ä¡Û?Þ]úª?·å[Ä¡ÛAGN3FGL J2356.0+4037@[íÿ`Ï‰À5ÏÃøÀ9ávÐ@õ"À;ˆô›GõÚ»…Q¹@6û{6D?û+¿K"ä¿Õ¨ ,g´g¿ëvàêfÔ?ÑT'¹ó£ž¿×³δÀAGNbll@·Hiã½PowerLawNVSS J235612+403648?ïþ¢	ª£­?6[çU×>Û?%ßg'"+Y?6[çU×>Û?ïÎûl·'8?ˆ)ø‹'Pí?x'I´:—ô?ˆ)ø‹'Pí?ï݃ž…'¥?qðK†dé?q>0Èåك?qðK†dé?ïÿõŸžˆ>͇»ô¢I>ÔÂ9/¯t>͇»ô¢I?ïýœ"_ü?AáC@_?7?v½–?AáC@_?ï#ª»;;?°ã.\5•K?œŠ¡¹`¥?°ã.\5•K?ïЖþ+6?|žˆèۙï?w´€öÔâ?|žˆèۙï?ïÿÇAâ<d?@"@k=>ü_4Òïœ?@"@k=AGN3FGL J2357.3-0150@Wb‰ۂrÀNËä€G¸üÀ:h_¿ƒ8.À;çCHT,¨¿»ù´PBýD@³±"
‰F@üªß'!U¿©J·'Ú¼¿èÀ/³ªoˆ¿Ö¯ƒÓV @¿ãk<P,,AGNbll@þ²-VPowerLawPKS 2354-021?ïÿLF)¯ý?¼Jñ?·æ?w7À4?¼Jñ?·æ?ïÅUƒ%u?–93‡©É?}U>{³Ñ?–93‡©É?ïÛßû0k
?og!Ÿ$"'?roYž¿?og!Ÿ$"'?ïíuj²ž?Iá:?m ?béÊ?Iá:?m ?ïþÝOÉ8e?#Ö,áµÐ¸?"*ÿ\VZ€?#Ö,áµÐ¸?îàbyOÎ?µÚбãÜA?¡ùØj,'?µÚбãÜA?ïÂÂ.'—?BW9_¯?~žèð<¡?BW9_¯?ïp0?ʦ?'Pü¼e‹Ê?'ùø
/‡A?'Pü¼e‹ÊAGN3FGL J2357.4-1716@Q¯3+¦ÀR†–ÿöÅÅÀ:~I±ú¹À;¢I
5
(¿ðz)˜Õ¤@I—ö×7_?ü×›£¿åàQ*¸e¿Ø'-˜‹ôã¿Ø,ßÌT¿Õé†lý?˜AGNbll@¯…¼£nPowerLawRBS 2066?ïÿf?
'u`b?>ŠAíÃ?
'u`b?ïօCŽ†?…#]Å[}û?t½rmWÂ?…#]Å[}û?ïçºX£Q¡?X
ܜ¯?hE§H·t?X
ܜ¯?ïÿÁ>õ'ÒÿPT>ÿw¤Q‰£>õ'ÒÿPT?ïþޛ	
ù?s'sóá?"OõD^!?s'sóá?ï`c³aIz?¡u4åÐ?"ó‰"ÖÐË?¡u4åÐ?ïÔ8dS`?wTÞ"èfÌ?uãÍÛBÃã?wTÞ"èfÌ?ïý†_nê2?/o1>q7?3Í®@?
?/o1>q7AGN3FGL J2357.8-5310@tz WŽ\ÀO~`X/lÀ9*i;,ü¸À;{ªÙ\þ?ñÑv—áނ@g%%ÿ@¤Ï_ÏŠ¿Í@&€ó/¿èh®\Ê0e¿éÛ7¯Õ׿èõI¯»2àAGNfsrq@Š06z—PowerLawPKS 2355-534?ïú‹Á­ô?J‰ð{Y¢x?EÐüªV?J‰ð{Y¢x?ïÌ}«ÄÆ?¨x"´1Œ?yÁ*`àmN?¨x"´1Œ?ÒË&?›ËûPA,?¦‡'Ϻ£?›ËûPA,?ï¢ÒæŸåA?h°9*…p?‡KFFØ£è?h°9*…p?ïûÖʞìŒ?D™†q°˜?@¤Õ'e,±?D™†q°˜?îû7¼¸`7?°5ËrP<? L"3ž"?°5ËrP<?íí­4V?¢C÷ýae?°""¥?¢C÷ýae?îs(·aß!?•+(ŸFÜÒ?¨Ít‡NXø?•+(ŸFÜÒAGN3FGL J2358.0-4552@tŽ§Ÿì™òÀQàÀ48À:
ÐW›ÈÀ;ñy¥Œ¿÷?ñ²ŠV@3¼ðáª@ïÕ`EK¿æîô´N¬¿ê8IÈuû¿äÎíöŠ'È¿µ"§?۞]AGNfsrq@'VøÔýó¶PowerLawPKS 2355-461?ïÿŽx~@ù?XE‰h?aâÅé?XE‰h?ïÏøݐ®'?IW
¸7Z?x'.
^?IW
¸7Z?ïÙiŸӾ?qLê:X,ó?sK?ÂìÜ?qLê:X,ó?ïÿüÓ¶Ý>´zCsZ¾k>¹c'¾r-z>´zCsZ¾k?ïÿ¹½À.H?eÞ[îÄÄ?›$p>?eÞ[îÄÄ?ï\ÚïOX®?®±´§îÅ?"d¢̸E?®±´§îÅ?ï¿!9ÐJ?áÒ>|l?€7±"^c?áÒ>|l?ïÿÍÍu5¯>ú\ýJT>ù4 ªn]>ú\ýJTAGN3FGL J2358.2-1022@Tæ@.Ä9ÀQDy î?À9ÿ`µL}‡À;ÛQk,žÄ?òYôèõ¢@é÷7"{¥@^ŀ'W³¿åãC;"ÿÒ¿ì7ä7ÍvÁ¿ï´xAk?ç€`'çαAGNfsrq@wžƒä%¯PowerLawPKS 2355-106?ïý'ÅS €?:ßå쇨?3qÕ¸Tî?:ßå쇨?ïÎÞiµÚ?Š–iþSÊ?xý´w§;?Š–iþSÊ?ïwõ‡¬Y?ˆ¯*qåî?'OWÊñ?ˆ¯*qåî?ïö°Äa!?RCb•Hi?Ržw|öº?RCb•Hi?ïûz
nT-?M14J¨)8?Bֈô?M14J¨)8?îw–<Ëk?¸5*-uåý?¨†œ2mhù?¸5*-uåý?—?PÅFCüÇ?§.°Æó?PÅFCüÇ?ïc.PÓà›?¡¶øÄÃ?"š5âP¨?¡¶øÄÃAGN3FGL J2358.9+3926@\"aùðÀ6NÚ_\†êÀ:DýòÿfÀ;¯&2™°@À‰£µQ[@½v›<ÜÕ@ªóŸõST¿âDè´¬<¿àÖÙI»h¿ïp J3'
?ì–Î( ÞAGNfsrq@ ï*ÀƒoPowerLawB2 2356+39?ïýޑŠd?<¿¦‡?1tÎ%Ôk?<¿¦‡?ïÒè´^í?ˆiî‡çÓT?vó˜Â­?ˆiî‡çÓT?#Æ?ƒGßgù ?‰¿t֖?ƒGßgù ?ïÿÿýÚ>ƒ>8§Èá"&>0máT¨r>8§Èá"&?ïöí§ã´E?[T×8±°e?R$¯ÇäFÅ?[T×8±°e?ï4…!HÚ?®œ0×+ì?™o[ÓF€Æ?®œ0×+ì?îÜ<š¡<·?š•dD'ï?¢<6SXŽ?š•dD'ï?ïÿÿ8Hµ•>¯¤¤#BÖó>˜ó·ã$«>¯¤¤#BÖóAGN3FGL J2359.3-3038@)iÄupÅÀS"x $ÎÀ9½¹Ì?TÀ;¶°ê7.¿àêìX@
³¿e=W@,7žÞ¿ç1Ro°ßS¿ÞlŸÖI£7¿áœ¿^­½ñ¿Øê|"îËAGNbll@¡ƧPowerLawH 2356-309?ïýwT#ˆ?8$ð>™bã?4G<t±˜5?8$ð>™bã?ïÓûÁ?Ž='"³)?v®(2«N?Ž='"³)?ïÕ[Ÿ
 û?sqÄÅ?°?uR0‰í¢ƒ?sqÄÅ?°?ïüôc®j?-‡íW+i÷?;]»ã2?-‡íW+i÷?ïù¨Í¿?PžYՅïH?K•\ãg%¿?PžYՅïH?ïy1*ÿ?£ƒÇ]<À'?Þ9ܚ *?£ƒÇ]<À'?ïRJû{â?ˆçwçÐÛ¼?Œ+m:Aϖ?ˆçwçÐÛ¼?ïÕ6?=i?nD™ùJ?uwäßs™?nD™ùJAGN3FGL J2359.5-2052@Lù>À//˜ÀS'*ŸæºµÀ:Nè},{‰À;ë?Íui9ÀLEÓÉÁ@»ž6aeö@$6ßæ+¿èûAîs ð¿Þ",æ½å¿áZ˜U²ö¿¤­ca4ŠAGNbll@¢†‡+JPowerLawTXS 2356-210?ïÿ ›þ?l·P>u?|åí•=²?l·P>u?ïÚuÑW9ç?)½pêÊù?rÅfA/?)½pêÊù?ïÙÆBD;?jó	5×|ý?sÞö®'6?jó	5×|ý?ïÿý¬œ3Z>°Ñ¦òæ]>²›Ð@yB>°Ñ¦òæ]?ïþ0Њš?+1|§ê}'?,ó$^‡Ð?+1|§ê}'?ïˆDQ`Z?–·Û°ÆØ?î뤌
€?–·Û°ÆØ?ïZӂ•é?‡ìºágí?Œ)K)©Yœ?‡ìºágí?ïÿÊQ·¤>þÅ]üF&>ú×=çc©>þÅ]üF&AGN3FGL J0000.1+6545@]lh‡¨ÖM@9Aâù^üÀ9ðÇô À:æåèðð?óÇî@
©ÛÖU@I£@Œb$¿ÜTX
ÇÉ¿æRGÀ*tj¿í$[ÒK+¿ÕÕ¤l†fUNASNone@'S@N¤©PowerLawnone?ìo´‡ a¤?¿<ç'õ
"?¼'[Âüòã?¿<ç'õ
"?é˜f‹Ê?ËÖçØÂ?Ë͞eӐÙ?ËÖçØÂ?좑¦õ¼t?¥¾2›¬Æ?ºërÈR`?¥¾2›¬Æ?êmSÜ\H?«,í—õ4?ÆJ°ŽŽß½?«,í—õ4?ÞÌóÓ÷¹`?Ш#±FE?à™†#P?Ш#±FE?Ύ,œàï?Í\é|¨>š?è\tØø‡Ä?Í\é|¨>š?æ˜XE*Eh?¶ã{em@?ÒÏOu«u1?¶ã{em@?ӗäTË*Ù?Ä°å蟺?æ4
՚j"?Ä°å蟺MIXED3FGL J0000.2-3738@u–'}keªÀR¼—žÖÜÀ:ÀঞdÚÀ<åS¬O?ÙÌd3ӎ@lþ.ϐ?ýÞ"?pq?Ã}¸X‡¼´?£ß!W tֿԐÞÎX¿ä½÷n®UáUNASNone@©À¨šu%PowerLawnone?ïþ}«@Né?&ÛPòœë?(%I
3zÏ?&ÛPòœë?ïÅRÙõ2?"6PSgv«?}pց'o?"6PSgv«?ïÓoã¤?q	 íê3?vwq;¯–?q	 íê3?ïº8ïúh*?côo[%Ô?qÄŒV?côo[%Ô?ïû·dEê?@wMÅD?A!Ékøþ{?@wMÅD?îÒþ9×<<?³Õ2À›B?¢Ð_ø‡<?³Õ2À›B?ï¶þ«N?;Š{^½?'@\1öD…?;Š{^½?î³¾Èʁ?¶Ž
Þð?¤ÄvNj?¶Ž
ÞðAGN3FGL J0001.6+3535@[êU!š"{À:0AÿŽÁÀ:iTz«—ÉÀ;Ý+€À…¿þ³LØç@ÒèDÍdw@ÍÞ?eñv¿í"O'…€¿×òp'@ƒö¿äSÿv¿Òw:/aÿUNASNone@'A¤¨ÁUPowerLawnone?ïýQMa?P:€÷l~z?7wº[ÃÃ?P:€÷l~z?ïщ9qˆ%?ˆØªðf×f?w;cIû'?ˆØªðf×f?ï€^¶*G?‰³Iz½G?èRÍÂJ?‰³Iz½G?ïÿôθN)>Ô@®0åܦ>Öb^›UÍG>Ô@®0åܦ?ïöòðDm?T è[?RifpÙ?T è[?ïCíucÚE?­bSÏci­?—'QX¬!X?­bSÏci­?òƒü¶?›æ^¹áÈ
?¦Ç Öfª?›æ^¹áÈ
?ïþ'¦Qҟ?+û×["1?'՘¿Gô?+û×["1AGN3FGL J0002.0-6722@sb9-Œ*ÀH‡ê=ö۔À:n»ØˆÂ²À;çŽ
^v?ÔQn:Mâ@¦€®ç	?ÿ#?B‹?·m¸\Nj¿àºj­{^¿Û"Ï2r¿ßÞqƒ±êUNASNone@£Era|ÚPowerLawnone?ïþ:%s`?#rh—¥[Z?(\F¿M?#rh—¥[Z?ïÌbë†?"÷ؒsx?yÎñ•Þ?"÷ؒsx?ïß?˜Ç6¶?j7ámk±à?p`3‡9?j7ámk±à?ïß[é÷f?QiÛXÞ?õ?pRr«P ¶?QiÛXÞ?õ?ïý²Ùd=u?1L›M~?2i65 Šf?1L›M~?îùu©Ç±|?² •P"›û? h¥fô"5?² •P"›û?ïÑÈè<?xÁŽã*¯É?wó౤?xÁŽã*¯É?ï+Hʍò
?ƒw<"6!L?š–æ³i(¬?ƒw<"6!LAGN3FGL J0003.4+3100@[½³R¨CÀ>¾¾zúr"À:v,­5À;à/Q&cA?ÑGˆ>Rv@
6v5ƒ@nB@p…¿æȼ¦º¿ãVîÆ
ª˜¿ìžr"Šq¿ë÷[DŽ—UNASNone@äz–¼PowerLawnone?ž–"¾?´ ÄLžßÂ?‹–ØZZЗ?´ ÄLžßÂ?ï‹	¶Z?—l¨p¡?='c˜¡d?—l¨p¡?î™C'®?"CK\´[É?¦n®©30'?"CK\´[É?îOþŽ¢?!(S72è?«LJø?!(S72è?î¿C"zºm?ª'"þ†?¤ÍÚ'5?ª'"þ†?ê}:¸±?ȓŠQÆ`?Æá;Ð?ȓŠQÆ`?í.#n;"M?¥ÕÂá-ÛD?¶ŽäŽ#]—?¥ÕÂá-ÛD?݁żQe?º6‡³_ŠÌ?á?!×sÍ?º6‡³_ŠÌMIXED3FGL J0003.5+5721@]Š	ÞÀ¥yÞonÀ9ó"#]ÓÀ;…KQ7*9?ã,%2£v@€ÎۚÅê@vç?¿³Š?ïóšÇ'X¿ääëÿd.¿åÌ3Õoˆ¤¿â¾j}£ÊUNASNone@ á|ÚQPowerLawnone?ïôñU\Æ?lœà¦}?VU'
'?lœà¦}?î=6ÃFÍU?·Š¢
`?¬,"Ë"*®?·Š¢
`?ïhØeԒ‹?ˆ§©§J÷?'äóEm®•?ˆ§©§J÷?í°…¯_‡-?"|9µ£þ\?²{҅qº?"|9µ£þ\?ï¦[S¸¹Å?e@­Œn?†i+aò­?e@­Œn?åüàõ–?Ï¡;ˆ†¾?ÕÀ?àÓ?Ï¡;ˆ†¾?톸1ÕÝ?«™¶{Ðс?³Ê?ïM8?«™¶{Ðс?áÎ;ßv"ÿ?¿®ž…ß?ÜcˆAÖ?¿®ž…ßAGN3FGL J0004.2+6757@] •þÚf@ùÛ"Ðå`À9&ÀÀ:×t4…BÊ?õÓ.»ª:§@fyHì-@ù…±;!¿—è–¤>/³¿éì¶¥K²¿ålÙ¿pæ¿ëN§.œdiUNASNone@"Ár{²þÅPowerLawnone?؏Ë؎ª†?Í®'ûnj?㸸ª½?Í®'ûnj?Á®Ç&"\)?Ät1Ç£Ï?ë"N6whö?Ät1Ç£Ï?啮ã'ÆÄ?²}H1ˆhc?ÔÔ¢8úrw?²}H1ˆhc?×ã 	0'?«"|ç@ÈE?ä|Ž/ûg·?«"|ç@ÈE?Á(üüP¯?À§'¨èÏ?ëµø€ÀëÔ?À§'¨èÏ?£"Ûøu?³^~á=[?îÇ¿'ûÀ€?³^~á=[?כn¬`?¸"Ô%	9?ä2H·©Ïó?¸"Ô%	9?®µšiq_?"•MVPî?tåÊ?"•MVPîMIXED3FGL J0004.2+0843@Yæ^NÜÀJ.ý›¡²À:‰Ù\'HCÀ;Ü=TeF¿ÎJ¬)FÔ@ƒš›ø@gN``=¿è)þ_R16¿Þ'&ˆªÞæ?CC瘿ëÜC·(ºxUNASNone@¥•b¶®}PowerLawnone?ïèâ{Œ?f
d×lü>?g…(H˂?f
d×lü>?ïÏU`.¾Ú?ŒÒŠcâ É?xUOÝ¡Òì?ŒÒŠcâ É?íáA¤©Ý?¡'/æî#C?°÷Mñ"ã?¡'/æî#C?ï÷
Ù?@˜uڗ¶0?QäKŸÙO?@˜uڗ¶0?ïÑ8D,?y¯o˜®"?wcÝÙ½0°?y¯o˜®"?ï'q(aH?±±RKÓóE?›ÚõŽÊÏ?±±RKÓóE?휏d®Í«?¨P҉ú_?³"Ù?¸,?¨P҉ú_?ïÑC·dÛ¢?uU&!x²Ü?w^$2Å;<?uU&!x²ÜAGN3FGL J0006.2+0135@Y¡ß¹8›ÀM¥ÿ¼ä!}À:gÇÐ䉂À;åÅÌ'‹_¿üuB¿Ã$@§¡ïÿW@~Å ]®¿ãÙCӔg¿â>$A‡¿ä§³ª*Ð'¿ÙJµïˆUNASNone@œ?ø7´¢PowerLawnone?ïþàÁÝk½?!#"Íæžù?!óឺ\ú?!#"Íæžù?ïÒÛ¾›ö?Ì>qþ?vö' ²Ó?Ì>qþ?ï×í@	W?goƒ¨‡?t	_áMH™?goƒ¨‡?ïÿ÷Ædl«>ÌH¤î£€[>ÐsK¯5ÁË>ÌH¤î£€[?ïýá`òLþ?/mü"ð‰ô?0ôøí#*u?/mü"ð‰ô?ï;d q,Ç?±^uÌ_êv?˜"kø¹Ÿ$?±^uÌ_êv?切YNe?"^¸Q©?…ßé³X´?"^¸Q©?ïÿ>"îž?ˆ´¦6|?-b3h¥?ˆ´¦6|AGN3FGL J0006.6+4618@\ºÚQÎÀ/»µà÷üüÀ:4š"U•^À;µ/ê©¿²¡¿ï‹ìò@èé­@VŒ?"鬿ëªü ¶*¿çùÖŒ
˜¿æ÷/Jàè?ªƒÉ<Ž@UNASNone@"…<¹#¢œPowerLawnone?ïþOwr¹l?Bm±H¥5H?+†÷9O?Bm±H¥5H?ïÄ{,¾q?Šƒ
½Çl?}ÀB`ß\?Šƒ
½Çl?ïÊj| '?ucí<½KT?zÊÁ¾&šâ?ucí<½KT?ïþeoµ3m?WÏèLJ?)©Œ,Iu?WÏèLJ?ï÷FöM?]/iÒ½Ø?Qr6F?]/iÒ½Ø?îÙàAQa¥?²ŽLr?$¾?¢aû졳¬?²ŽLr?$¾?ï6•9§Zf?"mEjÒ¸?™-XÂ}­D?"mEjÒ¸?ïêž,Pk?c,Éô©€?eèa½²"?c,Éô©€AGN3FGL J0007.4+1742@[<ÝÖàLÀEô™÷LÀ:kå˜u­+À;âƉ¼­¿ÌûÛqïö6@ºS«x¿.@~á`'¡°¿ãøÏE^?¿äl¡¡¥¿åx¨åx&¿Ý@—UUNASNone@"^OAò×PowerLawnone?ïþ´S.PJ?'W£ ›¥ê?$ºÊËqÏe?'W£ ›¥ê?ïÒ>éAD?Œ
nçëì`?và‹zÚØ!?Œ
nçëì`?ïÊtNA½¡?lJÔSÅ ?zÅØè+'?lJÔSÅ ?ïúLq¯?1Ò/†¯ë?FϖÙ8.d?1Ò/†¯ë?ïúvn­n?MnNH‰w½?GŠ%·t'?MnNH‰w½?ï5£>F?° Mª@q?™K»¦Ú?° Mª@q?ï#!så×?–@ï1Ç:v?››ÑšKw ?–@ï1Ç:v?ï¸<!÷Õ?uwä_ßèI?ð÷†Ú.E?uwä_ßèIAGN3FGL J0007.9+4006@\~‰ô
(xÀ6Ø@žUÁÀ:[	Pá™ãÀ;Ï®KØE§¿•Yl‹w¥@Xö§¼@4p yr2¿ÎBœƒj€¿é$íú]Ãn¿Ýn‹ðò›¿âÝ«{]2OUNASNone@—'|í'hsPowerLawnone?ïÿG{ó#?fb;d†ü?ˆÙ'Ü·?fb;d†ü?ïÇRÃ¥î?ìWª×q¦?|Vð$\U?ìWª×q¦?ï͟ü<ڄ?w–ux)=Û?y0ÈՍæ?w–ux)=Û?ïðÕݏ	??BwX€è¯?^TE`_ Ú?BwX€è¯?ïü$±:J)?E§Q¦Y?>Úv¶Ÿ?E§Q¦Y?îö³³%?°lâra­€? "ÔÂ;X¯?°lâra­€?ïA^¨"Û?•Ø¡¢7ß?—Ô*ñ Œ?•Ø¡¢7ß?ïl¯*Ðc?~î›rB'Ó?¤Ô*ýB?~î›rB'ÓAGN3FGL J0008.3+1456@ZënÀY!ÀGT<}^ÐpÀ:W´üÀ;Ï÷1$e:?ÜÉr¢éO@PM7–DP@(	_Ð=¿ß¬Ýƒ€Ü¿áqK²0n¿åT†e<ù8¿å£Y
ÄeUNASNone@'ñßö"FPowerLawnone?ïùåe0A¢?Xk}¦Å¹J?Hjj'æ ½?Xk}¦Å¹J?ïŸ.À¸?í•É ?ˆ4PØÉÙ?í•É ?ïpÕ}º?‰²ã÷ɖ0?'ý|áି?‰²ã÷ɖ0?î†~œ"*?†,ÖB"nk?§˜3^_?†,ÖB"nk?ï`¯aâ?š¹àêå1?"ê
¬YÏ?š¹àêå1?ëÜáX†:'?ÁL·Ç5?ÀŒzçb?ÁL·Ç5?ìH0ÔÅOç?µ/ˆgåå?½¾yYՀÈ?µ/ˆgåå?ã£]µ'Éq?µmU†Ó?عD"Úm?µmU†ÓAGN3FGL J0010.5-1425@UbMÒñªÀR‡&k¤"ÉÀ:"¢ïƒ°úÀ;þŸ¹™ê?ðÃ?ó`	€@#v4åç@w_»ýG?ï÷"ÁÄO¿åä6j—šÞ¿èŠ(‰¥Ên¿ïÿ†S>ÁUNASNone@nÜ=îxPowerLawnone?ï>4†D}3?£WükJý?˜9o:ßõ«?£WükJý?ícªXrv¯?»^›Æ|??´â­=H1ˆ?»^›Æ|??ëWJfwû‡?©ÐÔêä¡?¢Öf æ?©ÐÔêä¡?êÎKWlM†?¢÷=$'ñn?ÄÆÒ¢NÉè?¢÷=$'ñn?îÀM.ÿ>[?°DÂ|0?£û-œ~M?°DÂ|0?æâZ®ãC?Ïb	Gb¦?Ò;J£9{?Ïb	Gb¦?å2ý«"?¹]¶ͅ
?՛Îö¨Ø?¹]¶ͅ
?Ý3?Tv]?·‰u pAi?áf`UÄòR?·‰u pAiMIXED3FGL J0014.3-0455@XåÄØì–ÀP†"&þrÀ9ÁÉ@PR(À;råB˜I?¯ZP ²Z¹@÷ä÷»ãÆ@MŽÆ,¿ãVaHæ¿êx.ÉRU¿àhà1®y¿ça6+¾¨OUNASNone@Ž#Ÿò䎊PowerLawnone?ïûOl#ê–?"²¢¤71?BÂP	·jÜ?"²¢¤71?ïÎ}ôD"?'S%Ø0ø?xÁ½þ+?'S%Ø0ø?ïååõ4As?jÉ
Í
?j
Æ?-?jÉ
Í
?ïꜰ>:'?JZES˜Ä¸?ecO­'Æ?JZES˜Ä¸?ïÿwקò"?ØËåD×?Ç	‰<?ØËåD×?ïR-°x"?±q¤V7Ï?uºH9s?±q¤V7Ï?ï¾±¦«¥á?€m…'d?€S–EHSí?€m…'d?ïgiüëE?±ÈlÇOÊ?"ò¼òûe?±ÈlÇOÊAGN3FGL J0016.5+1713@[ÉÐúX÷ÀFlÖÓõ¶À:n‹†±_‰À;ß-(W7?ê	UŽIPÎ@¾¨×Ð@D`Þ<¿âŒ]`â¿ä¸—G¿íDŽ $ô½¿Õ°æØÍ®UNASNone@‹Ôˆ1&éyPowerLawnone?ïö+ð±®?c\ð˜oR<?S¨îÛ³ü?c\ð˜oR<?ïÂÚǦ1?gä'ÍÈ?~'œ!K»¨?gä'ÍÈ?ïiçÝç•?ŒDÑ]ƒ¨f?'Ãd"EN?ŒDÑ]ƒ¨f?ï-ÌZÐË?u"¢…µk?Œ4Œ÷
=:?u"¢…µk?ïé³é.µÔ?q1ö¦q»?fLµÍL'?q1ö¦q»?î8H«aåp?´üÍÉá…Í?¬{uIá©?´üÍÉá…Í?íåФr»‰?¢Ã‡,COÂ?°ÑzÜØ5?¢Ã‡,COÂ?ëaÖ!ì?¶5ë—!Ì?Âx§"y¼Q?¶5ë—!ÌAGN3FGL J0017.1+1445@[«úëÄ	ÀG¥‰›õ"lÀ:"ùdoÀ;Ô_rV_?ĬÌɔ*'@³0ÅŜ'?þ àÀt¤Ã?ïûÛµÔ¹¿Ú›j"ÍNA¿èÇú¼#\?¦´+]UNASNone@«ÿ÷škP±PowerLawnone?ïý+7Cìœ?9°yÈYE?6¦DŒÛW}?9°yÈYE?ïÐÊÊi?ŒÚÞ¸{"È?wýü®ˆ‡W?ŒÚÞ¸{"È?ï…À¬-?€ÊGåYz?ŽÔÿNÒ?€ÊGåYz?ïöˆ©Ì–?E«Ì[<®ˆ?Rî¬Âª'Ë?E«Ì[<®ˆ?ïôÎCDxU?YŒ5ä³\?VcyaÖ(?YŒ5ä³\?ï.VÃ8×ë?°ãrâ$ì¬?š5'—-4•?°ãrâ$ì¬?î…q‡4oÒ?ž2ۜäÊ?§¨ç‹Ýä?ž2ۜäÊ?ï‡V6 +!?­ï¾žž­?Ž*r~Ôo¤?­ï¾žž­AGN3FGL J0020.9+0323@[ªà"ÀMLæ¯ÌáÆÀ:Š£×
=qÀ;º™?׆d?Û±±=¥'@ù˳G@?ú=	þ±vZ¿ïöjÌ;?ïüÃ'I¿É§Õ"Öó¿Þx&ŸH|"UNASNone@¹<\)PowerLawnone?ïÿtg¹€G?æôƒg«?s	¼#å½?æôƒg«?ïËz4ë?H
ó݆?zBúSSFG?H
ó݆?ïáöKŸ¾?p6‹ò¯çç?n	´Û#²¤?p6‹ò¯çç?ïçÊq¨¹È?RûyV¸?h5Ž3ŠH$?RûyV¸?ïþÿ_C}?ú#©q¸³? 
Ô~f÷?ú#©q¸³?ï=#ÄM?²*˜FIw?œ¯Ø]?De?²*˜FIw?ï܎.è†ù?t3	 së›?q¸è˜Ë?t3	 së›?ï¶ËÈã*ª?tqÎ0E‰I?'M
·¿¯?tqÎ0E‰IAGN3FGL J0022.7+4651@]uõ׈²À/xpCßÀ:4Õh-À;ºÊá:B¿úŸ/¸ªUÿ@
"€`7£/@F/ßÁœ¿ë"Øz³ƒ¿â"ß½Y+.¿çŃþZl¿ïÿî¼zˆ÷UNASNone@|ፄM;PowerLawnone?ï%žÆ»L?«1¤G/"÷?›L'*NMº?«1¤G/"÷?ïÈí4@?Ž"nFTÉ?{þ‰PªÌ?Ž"nFTÉ?í(¨Í?¢†2¡¢Y?¶¿ú¿ñ"?¢†2¡¢Y?ïÿ(–;'?Ôg²Ã@?í4Á묾?Ôg²Ã@?îì²ø?¨ÚîdÙ?¡4Þ-B9~?¨ÚîdÙ?îþ±0?°Zœº¨‹d? ìô{
º?°Zœº¨‹d?ëÜ*˜ô?­_V½&¶?À³Uœ-Œ?­_V½&¶?ïázò˜?kñº,¸ ?n…õ¬P?kñº,¸ AGN3FGL J0026.2-4812@s¥í»YÝÂÀQ°J¶¸À:[7 '½´À<
Õ«˜ ¿Ù-jôb	'@ŠBÅøG@ù1~'¿Ú/õ¾*¿ÝOõd}¿äï7+ª¿á{Æ!ü™UNASNone@–q̈́M;PowerLawnone?ïý}ZYùØ?1mãüÿ£K?4.Q]-Ë?1mãüÿ£K?ïÓô=_?Œ}T§g±—?vùöÇä-?Œ}T§g±—?﵇…[?|ñuöÄÂ?'žþõÿ?|ñuöÄÂ?ïûŒ±\aˆ?-Á:܇Ó?AÍ9Æ]lT?-Á:܇Ó?ïûæí׫Å?AÛó®²;?@dHoÈ?AÛó®²;?ï?J›Y¸-?°|ñÏ,ý?˜¬˜8–V?°|ñÏ,ý?ï[Wq"yt?±§x?"•ÝhŸ}?±§x?ïÅS6Ÿ'?p€Á4«ìÍ?}V@|½'ç?p€Á4«ìÍAGN3FGL J0031.2-2320@Qà% …²ÀUŸS À:§H>]À<
àO`d?âêñ3ša@;7äs@ç`Kð?¬ûÕ¿ÜSÜÉ͜‰¿â—=x¨Õ™¿ïøô
Œ
HUNASNone@˜y#¢œxPowerLawnone?ï%µNUù\?›ˆ lÔa
?›IV6ø¢"?›ˆ lÔa
?î«ß}´?¸"Í|žI?®¥Bo6Ã?¸"Í|žI?멆€Ú}\?§P«ÃV›1?ÁYåü–
?§P«ÃV›1?먲µ¹#¼?¡'*·õ¶a?Á]5)q?¡'*·õ¶a?î·¿Z¯Š-?¢…¥€-?¤"
P»Ú6?¢…¥€-?è0SéÐØd?Ðm"%LsT?Ï>°X¼žp?Ðm"%LsT?ëùĹ?®•íŒÍé?ÁÂ"í?®•íŒÍé?Ýh³öÅ¢??¸÷Ø}ÕÏÈ?áK¦.á?¸÷Ø}ÕÏÈMIXED3FGL J0031.6+0938@\¶ñ€
|ÀJtîõÀ:.´iÿxÀ;»²åšùì¿ßçQu
›@
ãtÈG@Aë>":¿á‰Ñ¤fÀî¿ì€|Má¿â
N×æ¿ÄÃ9TyBÑUNASNone@",ã¼Ó[PowerLawnone?ï÷>ö_î'? .‡Ë™œ?Q'$¦Ñ±? .‡Ë™œ?ïÓçh"xË?‹µ‡n›TŠ?vK­õfŠ?‹µ‡n›TŠ?ïˆ
¢w[#?y=ÿ§Ü?ü—ioJ?y=ÿ§Ü?ïüŒ7RÉô?+€†Ù Ei?;žCMÔ*õ?+€†Ù Ei?ïÿ#ˆè"Ê?&éî{éý1?ŽëdþF?&éî{éý1?ï:½´½½?¯ÓƒÿŒ9J?˜¨Ipón]?¯ÓƒÿŒ9J?ïcŠ>÷?˜1ÛºéYý?³Ž¯¨4?˜1ÛºéYý?ïÊ!`;ÿ?tmòÒêûæ?zïOïܐG?tmòÒêûæAGN3FGL J0032.3-5522@sI輜$ÀNÆ6!úü‹À98ҙ•gÜÀ;ÆNóƒû?ÔVÆÚ´/â@ñ=ÐE'@2YÀe¶=¿×†Pn¿åÀ_±krj¿åþ.æ꨿ãú¹˜xÃqUNASNone@Œ[Î!–R½PowerLawnone?ïÿM
WŠ?!ɚÌOD?^MIó	Q?!ɚÌOD?ïÕ3‰'?ŒXù-]Ê?ufp1¡NÎ?ŒXù-]Ê?ïÆæàC?y'¢HLœ|?|žw*€?y'¢HLœ|?ïÿÛÄ{3l>àõ)õV‰6>òÌpüQ>àõ)õV‰6?ïÿ1Å01‡?ƒŠ!t[?ÇY´Âv ?ƒŠ!t[?ïF*qe?°&#Ϭ¿Ö?—=º°s?°&#Ϭ¿Ö?\ B?‰'Õuªáq?ŒÚ¨óø·l?‰'Õuªáq?ïÿ±½–'Ã>þî7|9ç0?™¢—>þî7|9ç0AGN3FGL J0032.5+3912@]¼ãÿï9À7ƒIàâiÀ:L‡È¶½—À;ظÙÐÁN¿ØûÒ4{îÊ@|ž©£ÒØ@'â?û˜'¿í–W£]›¿ä®Ús~|Þ¿à¹ýЃn=¿àFÊڐŸUNASNone@‡E©ûçl‹PowerLawnone?ïÿpnZ¯,?øíRôÇ?ò3ù½óó?øíRôÇ?ïË6Š´, ?Þ¼#ád?zdº¯ˆØ"?Þ¼#ád?ïÒ`¨wW?o–rà6?vϬ l?o–rà6?ï÷ iyc?;•%rè%è?QÇ¿'CŠ?;•%rè%è?ïÿ*ë;!ê?*ý>¤?¢™ê#B?*ý>¤?ï
ÖeZ€]?°>çrD´ô?žE3Mмr?°>çrD´ô?ïdžÝü ?Žj®Wh]?"l$E£…þ?Žj®Wh]?ï"ð(,Ö?ÿQ–5
?ŽÃöˆíæ?ÿQ–5
AGN3FGL J0048.1-6343@rø‡~äâmÀJ²D¿L±‰À:G./¾3­À;þö ƒ-G?óeø¸
"'@šUéŸì@Þ Z¾h?ïú$ƒíàÄ¿Ü®x¨‹ò¿âÓ2þ§L¿ê‡'éô'UNASNone@˜öã9ÀëîPowerLawnone?êGx®¬?'?ÅÜRs6Ñ?ÆâEOb?ÅÜRs6Ñ?ꊐҠ¡K?Ã÷ºGuF?ÅÕ¼µ}zÕ?Ã÷ºGuF?êgý_÷s?°Ž'hµ°'?Æ`ê€"5?°Ž'hµ°'?ècîdÕ 9?©2)!PKŒ?ÎpFl©?©2)!PKŒ?æ9{þ—äÒ?ÎÍë¹T¨?ӍÐ6[?ÎÍë¹T¨?཮ÕÒG?чÉ^>Šæ?ބ¢T[Õq?чÉ^>Šæ?ÙÑÎ/^£‹?Á3)7±È?ãèP®;?Á3)7±È?ש…>1­¼?µ·ÏíÖ?ä+=`ç)"?µ·ÏíÖMIXED3FGL J0049.0+4224@^'Ó"wÀ4tÙù9üÀ:mã؂µÀ;Ò?R%f¿Þo£78a¬@""^žñÈ?ü>ñŸêìs?ãˆ)ºc"£¿çÏÅ^)½$¿Ë÷W<쉿ÒIûÒ·ëUNASNone@·«Ýó¶E¢PowerLawnone?ïöëyÀí? .bÁz»?R)(y&K? .bÁz»?ïÇz6–®Ç?úpVÑ´?|B䢸c?úpVÑ´?ïâ¬_Äáœ?bý'‡Â"²?mS 'à"4?bý'‡Â"²?ïþNhÝ}ä?[—æh?+uȤ¹?[—æh?ïýäͬ>?7¢zø+?0٘ç8¨?7¢zø+?ïå.v´?°—}'`V?žcZ(¦£?°—}'`V?ïÑZDç]?x
ˆe…èý?wRÝ}3.n?x
ˆe…èý?ïôJC‰ÜQ?Q<ßYaí?Wky+€-'?Q<ßYaíAGN3FGL J0051.6+6445@^¼âCV–æ?þ3:ß¿À9†'•ùÀ;&±¥ÿÙj¿ÇùlŸÝÍÈ@MB¨ñü1@;ê€fí ¿âÃÔe>ëp¿â u¡<¿å®ò)伿ç:ӓÃõ@UNASNone@šÝ!|ÚQPowerLawnone?ïíiPV)?•g÷"EV?b–¯½qø?•g÷"EV?ï·öÅg?Š—"QÅ?'X–TK?Š—"QÅ?îŸÊ$?…Å®œ÷LF?ÝDTÛ?…Å®œ÷LF?ïæyª?Qúa²Ûà•?i†üh°Àj?Qúa²Ûà•?îs숡F.?¯i~k7Rõ?¨Á7w£k#?¯i~k7Rõ?î/07ç^/?¸$Tˆ˜jp?­üŠ?¸$Tˆ˜jp?íW…¬–??©½i`S?µCҙ"°?©½i`S?îó"Uã?•Soæ-K1?¦ ÎSK×?•Soæ-K1AGN3FGL J0102.1+4458@_;6;%pÀ1ÛÇæ³þ À:‰–Ob=ãÀ;å¡ÔÑ~¿ðV+57ð1@
§òz†Xõ@í@Š´¤¿çíô¬²•¿ìÈÒÊÆ@?ʈJ´%®]¿é®þn–œËUNASNone@™µ¶"Fs'PowerLawnone?ïüAå
ò?>ˤèŒ??åñéW±?>ˤèŒ?ïÉbõmªÓ?é91k?{N…A›ra?é91k?ï¸vVÑüj?~•-ñÏ>ƒ?âjY—Kc?~•-ñÏ>ƒ?ïÿiþ²‰;?
~ë÷ù U?À'.
Õ?
~ë÷ù U?ïö*͚8a?UŸ¨?SªeTÿœê?UŸ¨?ï‡"€Íg?¯§µƒ]¶?ž/
x}Y?¯§µƒ]¶?ïY<B?–'Ôž6é?œŸtÛçJf?–'Ôž6é?ïüœ‰t?Beç
Ø'??we_0¯?Beç
Ø'AGN3FGL J0102.1+0943@_Õ*¾ðk8ÀJ†«Oœ À9üÙ~‹÷À;¶Jt˜XQ¿çef#þë@
ÚŸƒéY@…*ÿ²þ¿ÓU3À™/3¿æ)"Á¿à<q—5Õê¿Ó14iØЀUNASNone@ŸiZu%FPowerLawnone?ïÿkÏ;?pÃõ† ?† Q¤ô?pÃõ† ?ïÕ7Œß!
?‹×'‰Á£?ud9{ÑÑ|?‹×'‰Á£?ïâpÞ"—?lÇ{àMù?m!öëÉX?lÇ{àMù?ïÿî€aö?íˆZŠ@²?¢8Qšw#?íˆZŠ@²?ïÿ(ø°Î?®bÛºò?üD¤Fü?®bÛºò?ïKzˆ>?®ƒBv9p¤?–¯ýÐ,?®ƒBv9p¤?ïÑØîKÖ ?zÒ\³$$6?wˆÇ‡'?zÒ\³$$6?ïôn2Hã°?Q&´¾Cã?W#›Æ.Ÿé?Q&´¾CãAGN3FGL J0112.9-7506@rÑ.Hè§ÀDøûüe@ÌÀ:o5·qñµÀ;ùRÈ#ð À°§ø¬út@
m…6‹,n@`ŸõÔ-¿çÅùÛ	¿æZÅkY•H¿áªú_à˜å¿ÙúÛö,äÝUNASNone@™¦Âø7´¢PowerLawnone?ïÿ
€~A?ö¨N§èÁ?Oÿ´VU?ö¨N§èÁ?ï×õ?Ôú?ˆ "o33?t…`ƒ9?ˆ "o33?ï弋=Ï?g@p™¬J2?jCtRDí?g@p™¬J2?ïÿÿÊPË>'ôB½ÏeÔ>zîÜf÷Ï>'ôB½ÏeÔ?ïÿ(Çö?+OVt
×?çߔ?+OVt
×?ïTúâe?­	é*)?•~`»Ôt?­	é*)?ïâ_ÝŠ±?q÷ÄÔz%?m #ÖŽ?q÷ÄÔz%?ïÿôØë¥;>â¡ À3Ë>ÖM¶;ŝ>â¡ À3ËAGN3FGL J0114.8+1917@`P§æšÔÀE¯ž¾œˆÀ:•k/ùÂÏÀ;âCæߝŠ¿âlä{%vm@
1_C1ƒ@{] :¿ëḯéÅg¿Ï·zn¿ä)nDÅñ€¿â¿#ì:È UNASNone@˜´GE8ï5PowerLawnone?ïþ"f÷?3Q_§Þy?/Ÿ:HøUµ?3Q_§Þy?ïÓlî¸&o?Œ6Ÿ"Ôd¦?vIˆ‰Ôª?Œ6Ÿ"Ôd¦?ïŸÄý†º*?'æZe-*?ˆÀ¨ Ik?'æZe-*?ïûSÓGš?0e³±;¥¬?B°´ä¥?0e³±;¥¬?ïøýÂ/‡O?Q¸jWÁ?L÷N‡¼*?Q¸jWÁ?ïAÌ¢Ÿ@'?°­†ØÄ?—Æk¨¨QÚ?°­†ØÄ?îÐÿƒ½B?™ìÃvݎ?¢ðcx¨ç?™ìÃvݎ?ï¸Ý&ê®?v†qSe?È¶K+у?v†qSeAGN3FGL J0116.8+6913@_L³åu:?@ߑæFñVÀ9xÓ³pÛ4À;04	t?ä§ÉJaM"@eQ5|¹@ à_Ñ¢¿æ` ÇJ×À¿ì°Ê!:§
¿è‹êפ¿ïýôf]›ÖUNASNone@Žó¡LìBPowerLawnone?ïÛ¥"
ñÛ?kœ¹ÓO!?r-oSfA?kœ¹ÓO!?îßÖiP?£s'î,O?¢™lµüJ?£s'î,O?î›F«Ç)Ü?•z>°Jþ/?¦K•EE0@?•z>°Jþ/?í>Ǜµ}¦?9·¦F'?¶	Ã!x+Ó?9·¦F'?ïdLm
kñ?'Ò· ÕGý?"vraÂä?'Ò· ÕGý?å0ü†Æ$´?ÏÏÔÚôi?՞òs¶—?ÏÏÔÚôi?ëȉ­N"r?®f¸½Ç?ÀÝÙJŲ8?®f¸½Ç?ÞȲrÕ?²°>¾ÛF?àü¦Æö?²°>¾ÛFMIXED3FGL J0127.4+5433@`3:}ªÀËDå^³À9êÁþ<±aÀ;t»ÑÒÆ¿ä<™$˜'@·ºt°@B‹ÿÓ	}¿ç]Ñ`¥•¿äÔºLA¢¿í–úNÔé?Ç z^ò\UNASNone@‰ä;â.]áPowerLawnone?ïû]xÖ?LOz_T?BŠÕw@½?LOz_T?ï¾Ç˜|Ûj?ïAÍÍ?€NÑRç…?ïAÍÍ?H=íˆ?·þ¸C7?Žœn²ª?·þ¸C7?ïÿG"'n'?f=v2â?
'ßÁøç?f=v2â?ïÚL¨¶SJ?vàÓ7r¤?rÙ«Å"®á?vàÓ7r¤?î§f§˜¥?³P€üã'?¥ŽI–b\µ?³P€üã'?îlƒ^Lo?œ™Ôã½?©?Ê9?œ™Ôã½?ïç@C«ë?lܐ}¨Ú¥?h¿à×ÐôÀ?lܐ}¨Ú¥AGN3FGL J0127.5+5634@_û
å6PÀÏbùÊ[ÙÀ9†}™ˆÒ¢À;V¶7_Þ¿ñîJ 	¶@åtìf;@°ª_d"¿á>ûù`(µ¿ì•
5üó¿åPS«‰í:¿ÊÑPŸGƒUNASNone@…¹x"PowerLawnone?ïþ&Þ³v‡?.¯'~S×ë?-'¼Ú#õ?.¯'~S×ë?ï¿
	Ȭ?ÉF°h"?€<œB]I?ÉF°h"?ïºeÀè×´?zz*·èP?fÇÙÖõ?zz*·èP?ïÿÛ´éx¡>暯0W˜ª>ò%ƒ)à³>暯0W˜ª?ïø8÷K?S"óDÃAö?O¿/?(?S"óDÃAö?î¥8…q]T?³ô× îÖ?¥¬w§2\¿?³ô× îÖ?îõbúîj¤?˜Å1Ì —Š? ©ÐS­
Á?˜Å1Ì —Š?ïý–CM݃?1zn:+.1?3Mä&=&?1zn:+.1AGN3FGL J0127.6+4851@`!¸'ú
À+(iƒQX¸À:ÞC핚À;¬RLÓî)¿üˆà¡bç@Ñy[á}3@•Û_⓳¿á¨Æ0o›¿æ«2œ›'Ô¿äH-û)Æ<¿è‡S@]¾UNASNone@]ÕfÏAòPowerLawnone?ïÿx{ðCþ?´õ	¤™ÿ?ð€ÈêY•?´õ	¤™ÿ?ïÆyn€ç?Ž@Ä¿'Ïb?|ÃHÖ9ÞJ?Ž@Ä¿'Ïb?ïì\7l•?f¾Ü(JÄ?c£Èrþ*å?f¾Ü(JÄ?ïÿö)n)>ͼg¯;¡ï>Ó­ÃÉ©5>ͼg¯;¡ï?ïÿs '$?àÎUå½?žfh²?àÎUå½?îú8´ì<?°sê|ÛÔÅ? \t²ó:?°sê|ÛÔÅ?ïØê(/ý?xjg‰õ_Z?sý‹å#?xjg‰õ_Z?ïÿ>Ò¬=i?"·5©é?%¢þKC?"·5©éAGN3FGL J0132.1-5340@rÀˆPœÀO4MUhÇÀ:‰š8ûÊÀ<¨Å†‡n¿áEÉ_ÒE@k~K4†Å@Ž#"ÅÊ¿†Ÿ
[sz=¿æjÉÍhþò¿æƒþ8ø¿á}ØÚ"UNASNone@"kVlô!PowerLawnone?ïû°%)ã²?D‰iª¤h?A?kÌpÕ?D‰iª¤h?ïÓøò^p'?Œn‹JԊ?v†Ùƶ?Œn‹JԊ?ïsÔÁû?†Z €*Â'?'…gÚñÿ?†Z €*Â'?ïø˜gÀX ?:äHz?Mža½î$´?:äHz?ïò½š)âR?]îÔɒ1?Z"Ëù2œc?]îÔɒ1?ï8Éÿ¬·È?°Þ0ˆš)?˜æÀ±8ù?°Þ0ˆš)?î"nå?¢Ú¶"|('?®oǺÉ|ý?¢Ú¶"|('?ïr—˜sºô?‡¼ó'æ?'­ìa7‰?‡¼ó'æAGN3FGL J0133.2-4737@q¿'»/ìÀPü_oÒ À:/Ùâ_À<Ê~=ó¿üšg<z.Å@@âH_@¨è?Äæú¿çÇoE»©—¿æ¢Ißô¿ìä
‡Z°?¸K{Íð}UNASNone@Ï¿ÆT
PowerLawnone?ïüÆT è?@+!ñcè?9Í]Aúñx?@+!ñcè?ïÖÏÚj¼"?Œ"«=çß?t˜ÙÀ?Œ"«=çß?ït-v},?‡xÅMLp
?'}ºLð~?‡xÅMLp
?ïÿùyËjo>Éé"õ>Êì2›Ò>Éé"õ?ïõ#K<G?VÇi0|;é?U¹i×(Ø&?VÇi0|;é?ïQˆÄñGg?¯Šü"á«Ë?•ÎçcŽá(?¯Šü"á«Ë?îÐÇ8–Òó?•\T¼0L˜?¢óŒxJžÈ?•\T¼0L˜?ïþ¢'"0?.›êz/c?%Öݾ`4?.›êz/cAGN3FGL J0133.3+5930@`pyåŸ,Àg±j4À:
ˆß72œÀ;i)¾?kP¿áÞÜ°UÙâ@f
uú®@±?ÿÊP¿Î¹¸|*?¿è9@ÔB¿ÓÌ8+¯J¿êwÎkûCUNASNone@¢h=Ùb·PowerLawnone?ïö³ž†?U¦O#Å}0?R˜ÂÒ͕¾?U¦O#Å}0?ïµ
Ö?3¿?'¼±ŸëZ?'½J~ùb1?'¼±ŸëZ?îí2:½?•6T†Ý,Ö?¡,ßÌT5?•6T†Ý,Ö?ïúÁÒVÇ?2Ѝ¨î.?Dø·Î‡¬0?2Ѝ¨î.?ïë·«þK?h˜?QѐJ?dHT!QHÇ?h˜?QѐJ?îV
bA`?·ïúÔf?ªŸ_K…ú?·ïúÔf?}·nt?›ñ
—ïÕ£?¥Ä!|¿?›ñ
—ïÕ£?ïÐ3S`ò?oë\`o¬?wæV9‰?Û?oë\`o¬AGN3FGL J0138.5-4612@q<w¯dÀQ0Ý)4­À:W'hr°!À;õo|ž¿â
Ô1£™«@
ŒŠâq¥@|äpùg¿Ó1{©Ñٿᇜ|
9¿áT¯baR¿â¹'£¹¶£UNASNone@ŸdÅ8ï4×PowerLawnone?ïþåçXœØ?ûRr­qü?!¡Š/Ô©?ûRr­qü?ïÔuù‡d?ŒkÁ[+³?uÅxÝØ?ŒkÁ[+³?ïÛYÐUîI?kÃn¶3[·?rSîu÷N?kÃn¶3[·?ïû<Œ(d?0úдZúä?CéeÐÕç?0úдZúä?ïþ6À§?)mž²â?,ž(<£E»?)mž²â?ïB;"™¦?¯Ý$B[m…?—¸~Ë@?¯Ý$B[m…?ï´W來?'žÊðÑ|F?'ê:×N~f?'žÊðÑ|F?_`Ón?tø6ãaÿ?€Ð'Á<p?tø6ãaÿAGN3FGL J0149.6+4846@`—*0U2aÀ)ûԌ´®ÉÀ:K8ãv\À;œ˜È¹AÖ¿‹#ÔÛX@šq¾3Vï@õ `]7é¿ê±®B•s<¿éªŸlRŸÆ¿×K4Õ'lß¿ãŠò¯+ôUNASNone@†iXy=ÙPowerLawnone	?ïÿx\C^
?º°ií"?ôyûøÁ?º°ií"?ï·S•ö™F?jT)v@?'+}Š:p?jT)v@?ïÙffømÌ?ev_*Ñp'?sL̑‡Š?ev_*Ñp'?ïáŸ¨¸y?SZúÐ}ÊÉ?n`óWG†õ?SZúÐ}ÊÉ?ïþ]
ô?3ÿ¾¹&?*/R;SØ?3ÿ¾¹&?î$i¾ý¾?´Ç£\ÚÚ(?­¹dpˆ%?´Ç£\ÚÚ(?ï†âj1¼?‰(·øå7?Ž{Çhã-?‰(·øå7?îï:SF?'No¡8úf?¡Ü]aИ?'No¡8úfAGN3FGL J0154.1+4642@`¿rSÍÝÀ-£Íi8À:DPXÝèÀ;¹—×øyú¿ñîW@َý@
Ð1Ü@j›`n)Ô¿çLܺß0¿â€w€ƒâ½¿ïÿËeªºå?ïýø£ë,3UNASNone@ˆ"'©"áPowerLawnone?ïüÎ=¡\m?DôÝABBx?9ŽÅ;{?DôÝABBx?ïÇ<Ÿ:ç?Ž'á…?|a°X©¸–?Ž'á…?ïˆ38͸?€pøõüoG?ùó*íZ?€pøõüoG?ïÿý$>´Ø>¿Û‹¾Ì>¶ß-·dU>¿Û‹¾Ì?ïã~S†ÔŠ?xcƬÙ?l¬Ÿ§?xcƬÙ?ï	ä²?°-²B£?ŸÞÞ|Š…¤?°-²B£?îe=ýš'½?x'M»b?©¬ "íè<?x'M»b?ïÿY"'2?$ÑÜßyât?Ý[¨ùÉ?$ÑÜßyâtAGN3FGL J0156.5-2423@i¿m	Ö¶ÀRÆÍÈuO7À:žr©jÇõÀ;äçW'Ž
?ÇÛ_¦r‰Ï@;-Ö'•?þ7>ÀZ#?à);Þ'"¿Û0š5ò¿â°¡$Ÿ¾ï¿ØdÖ°LUNASNone@¥—ë…¸PowerLawnone?ïÿSOæи?-­PòŠ‡?–Ä®	"?-­PòŠ‡?ïÒú"¯tÍ?Œ{Wxݘi?v'¶ɂ?Œ{Wxݘi?ïÞ4CS'?d‡rÍr?pñe÷f÷?d‡rÍr?ïïjx'-²?Fºù[Ù)?`•‡cӎY?Fºù[Ù)?ïþÜd…?ãk¤Ý¨9?"9¾D€À?ãk¤Ý¨9?ï0›ëÐÀo?±>¨™R&1?™ì'‰WŽ$?±>¨™R&1?ï¼ñ§;‡"?€2uûhr?€Ã–1é?€2uûhr?ï"3¾ðt?€w& Qä?Žó…¶×?€w& QäAGN3FGL J0158.6+0102@cpcŠ	ÀLÁ¯ ê[SÀ:1únƇÀ;Å;"ë½S?Ö¨j²@P
;§Ëá@wÑ߆7è¿ç2rÓ~¿íëMƲV¿1š°.¬G¿Ò'¹'Õ§‰UNASNone@‰Ý$Ý/ PowerLawnone?ïÿ¿½3–t>þm#ú¨f?ÃbÚà>þm#ú¨f?ïÒÛ!ñ?Œy=Ûè%?vúo·$œ?Œy=Ûè%?ïâÜn³ðf?f9.ã€âû?m#'€Iª,?f9.ã€âû?ïô†­·;t?A:GŸ€{?Vò¤ÙøO?A:GŸ€{?ïÿš^²à4?LS\Ri?	hD± ÌÇ?LS\Ri?ï:4#žÓ?®§`ùâQ?˜¹{Š…—"?®§`ùâQ?idŒ`?…D¡
¹ùw?‡Ý¥ªLƒâ?…D¡
¹ùw?ï؄©™i?iÅ6—Ìþá?s½«trû™?iÅ6—ÌþáAGN3FGL J0200.3-4108@p`ì"h	ÕÀQ…=ÈK^À:o×½Á—À;됝T9¿åþi0O@Å2í<™?þüÀZxœ¿ï¤Ew¶ùY?êv–§Ì¸*¿ÞaË.žW¿ã𝫐ÖÁUNASNone@«EÌcñA PowerLawnone?ïÿ\®ž×?/O"ÀR?j;¢€Ô#?/O"ÀR?ïÕ*ƒ®˜&?Œ5É(ej?uj¾.ã9?Œ5É(ej?ïè:®ýƒú?a–!SZš©?gÅQ.8?a–!SZš©?ïüÙ9™m?,ÓÀ0:+?960¸q$?,ÓÀ0:+?ïÿ¬Í°?‹"p…?j^ž"©V?‹"p…?ïGŠ'œÊH?¯íg)¸hÅ?—¯¯ÖRû?¯íg)¸hÅ?ïæ:†AV?oôœï—VŽ?iáÅi@ŠY?oôœï—VŽ?ïß3X`Øø?g¡))rÖ¾?pfS­çXc?g¡))rÖ¾AGN3FGL J0203.6+1148@b°r\=îxÀG§>›A:À9̚`hödÀ;lQÕµ©›¿v¸ŠF|¨}@üçá¦#@·SàQäÏ¿å]Y¸`·®¿êÝÍç½g¿êÙ0\áyÏ?Лü,XEUNASNone@ƒ" ٔ[PowerLawnone?ïøÙOçôÆ?wÕSš¸ÿ?LšÁltËZ?wÕSš¸ÿ?ïÓT…Š»R?ŒH֏l¸?vU½PŸÖþ?ŒH֏l¸?ïh&4r"‡?Œ<«EØ@7?'û9nL?Œ<«EØ@7?ïûGA¡Ð?:wî%©?Cúã‡ÛÎ?:wî%©?ïï"^5Ì?gõs¿`?`l¡¸OÓÚ?gõs¿`?ï9¯Oâ?¯íø=)[b?˜Ê×ËË?¯íø=)[b?î`´´ŽMÇ?Ÿ%Ÿ2m?©ô´·÷
‹?Ÿ%Ÿ2m?ï'J½¾g?Dɤ?‹mP†k2?DɤAGN3FGL J0211.0+1922@brVWûi˜ÀCÓ<ŽXÀ:%S'^²À;²V´A»Œ?ÀV
1tu@
µ4¢žûÙ@•€r+¿à`3$ª¿éN·ñH'%¿âoÛ
 ¿ïÿH¯
2ùUNASNone@Ÿ¾vÈ´PowerLawnone?ïú6ˆ¹]À?Fe=K®âÔ?G%ÝöoýL?Fe=K®âÔ?ïÃãÙr'\?Œ†<Ž‰l¼?~Z¥
þ?Œ†<Ž‰l¼?îÞÞñx¹á?'0¶-}?¢ì¿äå?'0¶-}?ïeŠ2ôI?u›¹:´µ?"N¹¦žG¦?u›¹:´µ?ï÷~¼ž`?TºÊ¶O?Q‡µoÓ?TºÊ¶O?îhá"ø±
?³û~šr"?©qíÍSg?³û~šr"?îñN3ü?¢-'_ºQ?¯pu@?¢-'_ºQ?éõ¸e®ýÑ?±nÇïÿh?È)iD»?±nÇïÿhAGN3FGL J0216.0+0300@d
\|ؘ³ÀJÌ~bÜn+À:§.~˜ŒSÀ;äȁäq.¿êàB&"èÌ@
!Í°!›@2@·¿êVbÉ_J¿à(³éãQ¿Ø2|mӇ¿ã7µeó UNASNone@©ù"¢3œPowerLawnone?ïÿfš"¿?сù"²ß?,´Ú€‹E?сù"²ß?ïÕ)õë?Œ2W¸pß?ukxƒ#Rl?Œ2W¸pß?ï炃†'?W´);ÝV«?h}|Bö¾œ?W´);ÝV«?ïþ»mJS?=TŸ–•?$G뉹?=TŸ–•?ïÿ@ìý?ٕ:>?üI —ƒz?ٕ:>?ïK‰´QßN?¯ÊPO0'Y?–ŽÉrTz8?¯ÊPO0'Y?ïÜÖ»õc?pžÑ¸ý?q"¢
ö¢?pžÑ¸ý?ïðk}Qj?WBB«-c8?_)m_Li?WBB«-c8AGN3FGL J0216.4+0507@cÓH˒:ÀIà{ÃŽÀ:v¦%™½À;à€³Æ ?ÃT_Èèf±@5–٠ų@ë"ßöu=¿ãêRn·Ä¿Òë"Ì
¹¿ìƒh¯¹8¿Ø¼anô™UNASNone@–×Ûô‡ýPowerLawnone?ïüWÝó¡ß?K³­ÛÒ1?=ACøX?K³­ÛÒ1?ïÒI=X™?ŒxrD¥}Q?vÛaI¢ß‰?ŒxrD¥}Q?ïŒiÃ8è?"%±‡¥dú?Œå8*?"%±‡¥dú?ïì̄RŠ'?O,HG䈵?c3{ÈòNq?O,HG䈵?ï鱅¯¾?n5v)'?fNz8䣲?n5v)'?ï4±:ә"?¯àßCëéÓ?™iجl«?¯àßCëéÓ?îsgê†,f?¡g6¢¬ÒV?¨ÉU	"ª?¡g6¢¬ÒV?îÞ1W?—ã"sñ½"?¢>C,†Ž?—ã"sñ½"AGN3FGL J0221.1+6059@`³"¦óõ0¿bÿfÁÄʺÀ8Ç`‹[uÀ:Ž¬ÇsÇx?ìy­
U@ºOÌñà­@ts@i|›¿è«¶݅,¿è$ŽßE94¿ë} ÝΰZ¿ïþ¾¢ù¥ÚUNASNone@"óNÙ‡+PowerLawnone?Þ±qoâo?Î{¼¯dj?à§wÇHÉ?Î{¼¯dj?èªy/Ž/{?שäYJ8?ÍVAÇB?שäYJ8?åH½ÆÊ@?¶žÉ²¥©ÿ?Õn"rk?¶žÉ²¥©ÿ?ç××{ì#n?¢÷W,ëm?ÐPQ'¹$?¢÷W,ëm?¿yyþô'9?Á,í‰Â?ìÐÀ!m¹?Á,í‰Â?ÌÆs"çÝ?ʐû+k#÷?èÎc>†	?ʐû+k#÷?ÚÊxÔÓ™?½Š¦a©]?âšÃ•–´?½Š¦a©]?ǂ1qœ¥?£¼Xj¸ <?ês»c˜×?£¼Xj¸ <MIXED3FGL J0221.2+2518@bjª¸¥Î[À@£
ⴖÀ:LÓP0šÀ;à { ŠO¿Ç±Ä'?N¹@
³9Ó¶K?þø…à19¿îÉôYo?à¹*,q£¿×SŠ^ƽr¿äÁ¿z÷UNASNone@ªŽbMÓPowerLawnone?ïÿ, >pË?¾æqÀ˜C?k÷@}?¾æqÀ˜C?ïÎ	Ÿø?ŒQ"¼¨?xûûCAÆ?ŒQ"¼¨?ïäWÞ8Z?`]ã¶úM?k¨!Ò¤±\?`]ã¶úM?ïç*®þ?S‰µ‡Ì?hïÕ¯WB?S‰µ‡Ì?ïþé"=E?+ù'5.y%?/gj€z?+ù'5.y%?ï$BÀw‡?°	$-©'ù?›w§èx
9?°	$-©'ù?ïÕâØo˜?vZ0+.À?uö÷›h?vZ0+.À?ï0ôùÅ1?‹ŒpÆy'?™þá[Ÿïç?‹ŒpÆy'AGN3FGL J0221.8+6138c@`®›¥ãSø?ä8찗âàÀ8íŒ- L;À:9GMœk?éñiþ÷A@O‹8Wà<@[Ê@«kÔ?ïþːü¿êÐÛøíDÅ¿åoKKq²9¿êõ1ÌńÉUNASNone@§œtã¼Ó[PowerLawnone0?Ѩðl©'?ф~7q?ç+‡Éž«8?ф~7q?î>nKsW!?´|⇿¿ƒ?¬L:)í?´|⇿¿ƒ?âd°Ñ ?¶{qÖhP?Ûù6ž]ßÀ?¶{qÖhP?íL¬ ãX?–⑅#?µšžûC?–⑅#?ÍKûè)†?Êéñîáœ?è¿íõŸ?Êéñîáœ?æuþ
N?ÌdÁ
KÞP?ÓùÅåc?ÌdÁ
KÞP?ÝåôóÔÅâ?¸+BÓ(s?á
†?¸+BÓ(s?ä¼Þ·Ó7í?´wèí€&?ֆBY%?´wèí€&MIXED3FGL J0223.6+3927@a¶¼œ#¸À4;>šo'À9Ì@Äì-»À;À¬ôÀ0Ý?ÙlÑYÏT<@õ"m/®C@:㟢J¿ä%,º°´¿çS$͔ɿ䝻Ýï½p¿åñè–	ŸÅUNASNone@‹—s¶E¡ËPowerLawnone?îöà‡Úþ?Æ.\šñÅ? '÷ŽÂP?Æ.\šñÅ?ï°ä‹§µÞ?Í7¤Þ¦|?ƒÆÝ2_?Í7¤Þ¦|?ﶖ\Xé?'ãP¶•—›?'Zxt˜q¾?'ãP¶•—›?ïnfæÀ?p@äâ`?'3/ú÷¬?p@äâ`?ïTç,ÁÌ`?¨ÁEXooß?•c`ç<?¨ÁEXooß?ífˆ¹]Àa?¸…ÍlÙ?´Ëº6[×x?¸…ÍlÙ?î¦1lë?¡ÉPVõÿ?¥žÜ熓V?¡ÉPVõÿ?ê€lR—?¨|BçH^?ÅÿãÎNµ£?¨|BçH^AGN3FGL J0224.1-1846@hŽu:>À/ÀPÇÖ¡aä÷À:t˜XPúÀ;á÷Š¸Û¿Ë›éɁ@
Ä)Ùî@3ìŸûÞ]¿âT³æÌÓ-¿éûAÝ΅g¿Õ+s¢JSq¿ècÃUÍ~UNASNone@‹ í\ú¬ÚPowerLawnone?ïÿ 
®?C!݁?üÀ|Ÿíx?C!݁?ïÒ³aýÝ!?Œ…B‰7WÍ?v¦Nù'Kk?Œ…B‰7WÍ?ïÝÛËB^?hŽ@²hß?qx>¦?hŽ@²hß?ïë2Ý?{?N¶­ÏW²?dÍ"ßUR?N¶­ÏW²?ïþcõë!?'Xˆ¢'h?&)Ã75æ(?'Xˆ¢'h?ï8,Û(?®onï>?@?˜ÿšvÛ ò?®onï>?@?$	8}?…uÓm…&‹?ˆT7!|Í?…uÓm…&‹?ïILñ[ˆ£?ˆˆ›Wz^m?–ÖaË÷åª?ˆˆ›Wz^mAGN3FGL J0224.4+1615@c$÷QÕÀD‹·¼]êÀ:M®ƒ5ªÀ;©ãîQÓ¿ðò€Á1@±Ê]0ݘ@=½O¿äý×p·ª¿åË¥Š¾Šj¿ã.z:Èl°¿Û7\.nUNASNone@™YŸU›=PowerLawnone?ïÿ¶Ô'éÒ>ø<êÊ*?JÏvSáá>ø<êÊ*?ïÕ&~¸(?‹õg³ˆý?uló§æ¼?‹õg³ˆý?ïëۓ9-H?j-Žq²ö¾?d$lŠY˜?j-Žq²ö¾?ïÿÆG³¯>ðE
÷՚\>üÜH0&§U>ðE
÷՚\?ïÿºˆ°î>ÿq!Î'ë?]ÑîǙê>ÿq!Î'ë?ïOþ«Ÿ´?¯†ÐßÄÙ?–*…*Dú?¯†ÐßÄÙ?ïÔZSnÎ%?y_›]th?uÒÖA¹µx?y_›]th?ïüäŒÜòµ?4y* d?8ۘîAà?4y* dAGN3FGL J0226.7-4747@p´Ú¤ü¤+ÀO«ud0+À:²Jj‡À;éï#8ê,?Ÿ´Ð!ƒý@
j´©ÀX@Yc_uÜP¿êzŸ6J¿é¯
Ñ₹¿æU·A ¿ãqÁt1UNASNone@v¯<!~|PowerLawnone?ïþófG<?(gæ? ɞ'Ø?(gæ?ïÍ,°&Ñ?ŒØ*.RL?yi¨d33?ŒØ*.RL?ï²~Ü õ?{ˆæru?ƒ`yÆÉ?{ˆæru?ïÃ:Oº°ô?dƒÇÃù?~bØ«F*?dƒÇÃù?ïýËǶ"Ù?4´p6™"‰?1¡Á¦ë÷?4´p6™"‰?î‹ý³¹DI?³‡ê!?§@$Æ#‰t?³‡ê!?ïÈçSÐ{?"#/Qs²w?œã^†™?"#/Qs²w?ìµG«Ì]L?¥ Bê±\?ºU¡œ?¥ Bê±\AGN3FGL J0228.5+8213@_"âëC-@3ÿ—þŽæ¸À:INþjÕÀ;ÖYjÕa?¼s¬h@
Èé>Èg¸@,( Z"t¿è§®K=§<¿äø'÷ŽÂ¿êë™ëñL«¿ä³°Šæ'UNASNone@w¢B"ßÎPowerLawnone?ïý«c4q?8œNÑb?2¤å¯Óé¾?8œNÑb?ïÇ~G_ã?†ìæ@é?|@Üx@Jt?†ìæ@é?ïª:Zç#³?yµ¡pÖ<o?…qi?WÛi?yµ¡pÖ<o?ï¥"mµï?l`j¹àH™?†·~d'"Z?l`j¹àH™?ïéíéõI?p(.M=q
?f/Ò¸˜?p(.M=q
?íÞIaŸ?·D/{_ö?±
·×$ó?·D/{_ö?î¨Íu'ý»?óֆFñû?¥s(¦VY?óֆFñû?ê$еBJ0?³ök(Xhì?Çl½*ö×@?³ök(XhìAGN3FGL J0231.0+1302@c¤pâÁ*ØÀEŽ'Ð(¡àÀ9ý«®o´À;hÞë0¿ðXþú~@À…Téz@b³ ~O¼¿çV]Ÿ˜a5¿éZ^÷˜c ¿àÀIcÌ-@¿æqâÌÀUNASNone@†Š$ p¸ÐPowerLawnone?ïÿП)Å>ð»àE*>÷°ˆóÿ`‹>ð»àE*?ïÕÀœ	X?Œ/ÝÏd½Ö?u~Ÿ"¾Ä8?Œ/ÝÏd½Ö?ïì&‹ÒS?TÐÙK1=ý?cÙtBJ'ï?TÐÙK1=ý?ïÿfCÖ¢?¯þ¿uwÕ?<ºŒü{'?¯þ¿uwÕ?ïÿÙs=(C>òvÕ"P>óF`ù"íH>òvÕ"P?ïOÀ†Ó?¯‡ø.ëÉê?–üÆ+‹?¯‡ø.ëÉê?ïÛƨy?p3'ÎMî²?r«»9çT?p3'ÎMî²?ïøE·wى?Eu†Ï¾˜?Né#}³?Eu†Ï¾˜AGN3FGL J0232.6+0646@dNÚfƒÀH¿‡iì-À9öKµ
8hÀ;µ"Ô7û?ë*¬K{I@@ÒMë@SáÀNå¿çŸ?åŒü¿æf ¾;x¿íkÝxG¿ê{çNz¯UNASNone@}Â&€PowerLawnone?ïÙÙÂ9Ý?ä6ìhX
?suVm¨?ä6ìhX
?ïdPä–d}?"(´ßX0<?"uãp£Q?"(´ßX0<?îüàøöì?""3¨l? 1ðlRþD?""3¨l?í=O0LŠ?'U¯™g?¶‡Þë.?'U¯™g?ïÈ,~…Žl?ƒ;º†È2i?{éÀ¨›"?ƒ;º†È2i?èð-£7Ž?șÙÌJ×ü?Ì=ûIs!Ç?șÙÌJ×ü?ì§dQ¨,?®mħ?ºÄÝr¿î¡?®mħ?Ý+òN]þZ?¸áx ¨5!?ájØÑÓ?¸áx ¨5!MIXED3FGL J0233.0+6237@`Ê8›R~@(ŠbÄñ6À9h>­º¹À:²pSO2¿ç¯`Å"i@…&ÉB~«@XL jÓ¿èl÷òaÔ(¿ç˜Oº}iã¿ì×1ú™¿ØÃîÓTUNASNone@Š<a|ÚQPowerLawnone?îmƒãÇ1¥?¼1¤ñD.?©'Á°þ¶?¼1¤ñD.?ïÁ-ú0ª?ŠžeA‰s?iá{lr?ŠžeA‰s?íæà
57?©ìÿôÌ®
?·(Èýp"Ï?©ìÿôÌ®
?ïÿX–!ȅ?	Iµo¼)K?í>ÕV]?	Iµo¼)K?íÝ(Ä3:?µM›g,½?±¹Ü@nk?µM›g,½?î­	'+êr?´°EïÈñ?¥/féѼâ?´°EïÈñ?ê	÷Ì;·?´ŒyКo?ÇØ Ïµ%?´ŒyКo?ïó'X€?T¥Å ®êÅ?XÛO8ÐÀ?T¥Å ®êÅAGN3FGL J0234.2-0629@f-ˆ¤~ÏêÀMf^ê–À:ëLÔÉÀ;ÚY§;BÌ¿È´• ˆ³@÷;á,«?ý¢~ðuô¿ºô¿§¦€¿æqô%‰Û?Ÿ÷*|'T¿Í†•'˜UNASNone@±¨ýó¶FPowerLawnone?ïÿUía0¶?aCòY¢X?BN`±†?aCòY¢X?ïÔ5Ê[?Œs±ìNî?uåìSqŠ?Œs±ìNî?ïáÛû?`'§Aì7?n$åÌ?`'§Aì7?ïýÊù…˜?\'C‰Å?1¨83É>L?\'C‰Å?ïÿSþ§2?Šî]ôÓ£?"ö'ØQ?Šî]ôÓ£?ïIûÊm€?¯çüïxu?–ÀŸÓ?¯çüïxu?ïÓ4}`(	?uúŽ(-ºÞ?veÁ9>±?uúŽ(-ºÞ?ïöàú:þ?IÒ8aš%?R>v|CR?IÒ8aš%AGN3FGL J0235.7+5647@aC¿rq7À	Þ×ü«·©À97BL«ª=À;KïW;P8?žô¸[ö@nȯ†Á@Û©Àƒ=b¿ç}D®-¿å¿SÞµ"±¿çÈÛ$¹=¿ìñډŠUNASNone@a ÏPowerLawnone?ï®5ÜA8?•p`<
/I?"rˆïa|?•p`<
/I?ï˜Ñ‹V?£[?DÏ?‰Ë'ÀO?£[?DÏ?
	Ä$?—ødEÈã¾?¥ÇO_c½À?—ødEÈã¾?ïÆy6z?`øƠ̈Ã?|Ã1g³òÑ?`øƠ̈Ã?îwwäEÂà?ª¾%;|B?¨ˆ¿ïTó?ª¾%;|B?퓽ÔÇÃ?º¼ÄòÅ?³b¡óë?º¼ÄòÅ?ë9_‰AK"?±šƒõÿ‡E?ÁÚúѲ?±šƒõÿ‡E?íAÀýê.»? u†Jú~?µñøød¦? u†Jú~AGN3FGL J0239.0+2555@bè¬1&éÀ>ö]9–úƒÀ:"Ë@ÒÎÀ;Êry\ã¿ÛºI˜át
@
[,µ•£–@~¸`¿é)I8òԍ¿è—›‡…¿Öïòª	±ã¿ÖaÀ~#¶UNASNone@«þ*~ùÛ#PowerLawnone?ïÿ^¤
¾?cõ*Sô)?+uSbá%?cõ*Sô)?ïÏ]IBz_?ŒxÞEí‹c?xQ[tdN?ŒxÞEí‹c?ïؓ#«"P?v®]ö~?­?s¶nF›¤?v®]ö~?­?ïúù	½]?2`ÞJLL-?DÏv¢‰å?2`ÞJLL-?ïÿ;
ç? —äÒ*?%Jz'? —äÒ*?ï+0_:Åp?°
ÕÌñM?š™ôλó?°
ÕÌñM?ï҇U¥g?{±cŹ;'?v¼U'›0?{±cŹ;'?ï¼Ô,p)?z´y)n±·?€üÊü#²?z´y)n±·AGN3FGL J0239.4+1326@cæ_ZÙjjÀDÙ5C®«zÀ:
¹üæpÀ;¡ƒB??±¿îÄ×,n•V@v­Aí
Z?ÿìe¾ö [¿ïMQ'Ì?áÌD' ñŠ¿ácH7¸dF¿ãwrt³þUNASNone@¨Ï\(õÃPowerLawnone?ïÿø[?ì{†n6?ödÉï>?ì{†n6?ïÔ¾¨ò§þ?Œ-ÚÛb¤«?u «lŽùJ?Œ-ÚÛb¤«?ïê
gœœX?`P=-%´?eò˜›½?L?`P=-%´?ïþõùcP)?øƒ4Pø?  eÞ	Qq?øƒ4Pø?ïÿn°ª¶?' 8~Íl?>b'?E?' 8~Íl?ïN–w¿îÝ?¯‰Hñ8üq?–-1™*^?¯‰Hñ8üq?ïà®jzáâ?s³ŸpÈeò?oQ•ÄVí\?s³ŸpÈeò?ïó
3¢ÍS?Ta°U:›?Yå˜6t[Ÿ?Ta°U:›AGN3FGL J0240.0-0253@eÓ0üø
ÃÀK>ýuâlÀ:T¢Bµ‡6À;ä™/ŽÃ?è™SèNL@­Ô°p÷@€Ì_iœý?ϧïâj\¯¿çWvÜL¿¿ïÔFxVË5?ìý["KUNASNone@ˆ0rGE8ïPowerLawnone?ïÿ3fVB¤?%	óiu$?"<p+4??%	óiu$?ïÔ_MîJ?Œiü^Œ?u÷Pv•~œ?Œiü^Œ?ï>{LÚ?'†;"fÉ?˜0–ÔYs?'†;"fÉ?ïþ—"J"?('ªÜŸ€?&†»"±ù?('ªÜŸ€?ïþãlÃÅ	?)@š\£
Ÿ?!É/À½Ô'?)@š\£
Ÿ?ïAêä˜y?°õf__«?—£p`yã?°õf__«?îc÷uº8Ã?œŽî¡q?©Àˆ ì××?œŽî¡q?ïænG†Q?yº³(æ›?ip'Ÿ¼~º?yº³(æ›AGN3FGL J0242.1-0534@fS—c^t*ÀKûà¤&À:jùYó']À;ãåÇo•º¿ï²	Û~Ÿ@½§¹íÍ@×è€\†¿¿é`eŠÀ°+¿ä.ðÞ¤æ¿âTÂÝé2g¿ïÿZ=†UNASNone@ˆÐ†¸ºÇPowerLawnone?ïüa¯_ž?<i6ÍE£ù?<ò‰mO*_?<i6ÍE£ù?ïÕ³ÌS]Ô?Œ.ÖUøà?u&èÞú?Œ.ÖUøà?ï‰BjÍm ?€«¼;ñüê?¯eZc(?€«¼;ñüê?ïÿ,'ô?s©Ö?Üx¯ù?s©Ö?ïý•AºŠ?6Œì҉
?3UøO,(³?6Œì҉
?ïO!÷L?¯5h}Óü?–v™¬'?¯5h}Óü?ï0'6-?")J¸F>9?™íÙ:Xn?")J¸F>9?ïó)‹û²z?RUýÁlŠ?Y¬çÌ!í?RUýÁlŠAGN3FGL J0244.4+4745@a»C¬ÄðÀ%Ø?³t63À9ە+uϐÀ;©V)Ø@ž?óƒ#Á%NÄ@]¦^y(@þ€[¯ÿ¿èN›c?·È¿èÚç¤m¿í'<«WL¿ïþ-€IoUNASNone@|õòÅz%PowerLawnone	?ê="á?Äq`G1(?ǧ©ù°}?Äq`G1(?¿Ì N‹ö?ÅÉÑãÀŒÖ?ìkö..?ÅÉÑãÀŒÖ?ê¢,ÿM¹­?«'
ƒR	¬?ÅwLÉJ?«'
ƒR	¬?Ñ|.äw—?§pX˦º?çAöhÄ5?§pX˦º?á¥å5?Ѐ0ïÊ?ÝØ´5•ýÈ?Ѐ0ïÊ? NÞ8ɹâ?¶°r@h?îû¸'?¶°r@h?äÛŠ)å?·‰ÂÁ±Ø?ÖüHë¬5þ?·‰ÂÁ±Ø?"Hn6r
'?~)õfÝÑJ?ïe¼ŽLo«?~)õfÝÑJMIXED3FGL J0248.4+5130@a™
9À<ù…'À94´7ª'À;Oº*2Ùq¿Ð籺¢¨·@ûD¸Ã+@‰gÀ-­?ÆáëRôš¿êEØU'_ü¿¼e"¤7,¿áW£UUNASNone@¥ÓåãS÷ÏPowerLawnone?ïïtWä¿?‰è
‹†ç?`‹©8IV?‰è
‹†ç?ï´@Ž\ñë?'2‰²IR?'ïÜaŒWR?'2‰²IR?ÞüáN?"/®À†'?‰]HQõ¸v?"/®À†'?ïì÷ý¨ø?PÒ.;̼¶?c}Ϝ?PÒ.;̼¶?ïíšÝ¼^@?fûP«WžÛ?be"lÝ ?fûP«WžÛ?îNâñÒ?Ó?µ$Îw?«Ðç'…Å?µ$Îw?ïRV"×Û?'MEüÛ?•µ-•_?'MEüÛ?ïxܱàüô?…µzN9o?äiŘ/t?…µzN9oAGN3FGL J0251.1-1829@i;ºKâÀN•6½+oÀ:¥?CÄÀ;Ã}ºŠ?ìG>^ú%9@
b›«—ž?ùëÿ0ø?ïÿ9Ã^ÿ¿ïÿô	N*?ïÿÀ¤Vt¿à¡âDrªUNASNone@¸®÷KƧðPowerLawnone?ïý‡8b?7^Â`‹öÜ?7kƉ«¶?7^Â`‹öÜ?ï½údžç»?•¿Z)‰iµ?€NƒC?•¿Z)‰iµ?ïmB–'Ÿ+?Á*ñßð…?'W­7œ~š?Á*ñßð…?ïÐ×¥\µ'?uoTî*X?w"-:øß?uoTî*X?ïþ'€ÒÎ?1žåмȑ?-Šw#qâ?1žåмȑ?îÚÇON"?´¨Ù¾dä?¢SŽ|Âä»?´¨Ù¾dä?ï!—Î	Û?•E,O¬J'?›ÜÍ	®`˜?•E,O¬J'?ï֐†Ï?…zǾ½aí?tó7ϊüM?…zǾ½aíAGN3FGL J0254.2+5903@aDèh3Æ¿Â6év&À9Rk–QÀ:Õf££×?w0Éraˆ¼@­ºÛ³šw@D¾@Bo¿ä¨ÞI昿ë+`Š.m¿íµûxT?ÔÕĀ€¡"UNASNone@ˆø«¾Ê«ŠPowerLawnone?ïèß(*QÉ?t…²'+è^?g ×ÃÐ>¼?t…²'+è^?ï³pûô5O?"<[ó=F?ƒ#Á0&?"<[ó=F?íÿº®G?¡¤=?.FÃ?°/0tÃ?¡¤=?.FÃ?ïülÞ¶ÀW?5<N2Ï-?<™	`䔚?5<N2Ï-?î[°éR¦?±…²µ¸?ªG$òF¼¤?±…²µ¸?îþØô´"?ºAGyCì?®°t$SÂ?ºAGyCì?éúùªj;!?·BnÏsr?ÈVW|?·BnÏsr?ï£ßâæó?‹"vÔy'´?‡?CÖ§>?‹"vÔy'´AGN3FGL J0258.2+3555@b¼§›ºÜ
À47ÙUqKÀ:({_ïJÀ;¯è?ïÚÀÓ$‡É¸p@
†ú·Šñ@àÄ *í¿¿éÃG†Yÿ¿ä {Ó·'¿ïûbd¬°€?ïÁ˛R	UNASNone@ƒúáG®PowerLawnone?ﵒ²ä]&?¶ù¥›K¯?'›SNwÚr?¶ù¥›K¯?ïÔ»ÝÕø^?ˆ+´OÃÜ?u¢6 ?ˆ+´OÃÜ?ïˆ<̱kj?ƒêšy¦§¥?ðÌÓ¥%‹?ƒêšy¦§¥?ð=íkFÓ}=Ã˼öÈ|=íkFÑ.¹T?ïä,ë¤
?tò£ÔŽ–?kÓvû?tò£ÔŽ–?ï@é§yG?­Áƒêò?—âË—Å?­Áƒêò?·C+V?˜b®g³£?¥4ˆ]®?˜b®g³£?ïÿÿû´}>a-W칂F>A…¶Ï¦[>a-W칂FAGN3FGL J0258.9+0552@eW¡"úÖËÀFk	cV®À9¶3ßWÀ;†!È`?ákÒ]Ä_@
KYN$ü@ÿ9À@!ƒ¿à˜[êȜx¿Ýìß@0¶p¿á+µ¹=s¿æÛì4£"UNASNone@ Åóݗö+PowerLawnone?ïûD¥²'Ë?Z³»¼(Ä«?Bíj(²Ì6?Z³»¼(Ä«?侀"[[	?|i+G?…"ðu¡?|i+G?ïµ»wS¸?€r2̬Ô?'º-Ù½Û?€r2̬Ô?yXí"?yûÖ
ü?§4(gŠÒ?yûÖ
ü?ï×vŕ\.?y 
 ¬OU?tD4àò?y 
 ¬OU?ìé\Tê"?ºJZ°ê\ï?¸µWaO?ºJZ°ê\ï?î‰Y>þð?¢Ú¾Ñ,E?§jl+÷ý?¢Ú¾Ñ,E?æÛ~¨?¬vø¿ða?ÓæIÃȱ?¬vø¿ðaAGN3FGL J0307.3+4916@bAcÀB@TƒæÀ8ö"#—µÀ;KÒ®Že?Ù¶ˆ™'j
@ÕwQÆX@ÄÀ¿¿ãתˆ+µ¿Ú"ì¨y?¿åʖ;T¿ØË´¨'"nUNASNone@žÕ*™1PowerLawnone?ïñ(1€W?Z‡P³£
g?]¯mr·?Z‡P³£
g?ï¤o]Rbñ?–ѪN•Ø?†ä(µ¶Å?–ѪN•Ø?ïRm?®yÉ?•¼'E|ì?®yÉ?︮6Ý?fc:Ö?ÔX±ðÇ	?fc:Ö?ïKÀ‡2þt?•V§`êl?–‡ï0•Š?•V§`êl?톏Õå>"?¹|ŠÀzé\?³ËRÜñ?¹|ŠÀzé\?íWZ«-|?¦û‰5&?µG5,^b?¦û‰5&?íɡõ¥?¥7k–Åât?·i±¥
-Y?¥7k–ÅâtAGN3FGL J0308.4-2852@lÀ6âëÀMèÀh ÓÀ:Š7"D[À;õ½
·éç?Ѹg¡5+@
¹õ¯š@Kª@ýÁ¿çCr-nù¿æ&ÓØš¿ÚÀÇ2p¸¿ïÿNµxOûUNASNone@ˆ(è]·k<PowerLawnone?ï𿛿lE? 0íðŸ??^€Éuô? 0íðŸ??ïC±û»!Õ?šl-ÂßLÒ?—‰ÀÃ/g?šl-ÂßLÒ?ïæõ	?Ž¼ŽN'ym?ŸÝÃ3(Èâ?Ž¼ŽN'ym?íYlÉ4šo?˜Îöš<
?µ4™µR	?˜Îöš<
?ïôdw½•'?^ž¦¿·ƒ?W7Ä
­ˆ?^ž¦¿·ƒ?ç7ÅnM?Îìbã¾Å'?ёÚu#e?Îìbã¾Å'?î˜eØÞO?œàÐ{2DY?¦y¢vjž?œàÐ{2DY?Þãª4	?Áß-jFp?àŽ}*ðeû?Áß-jFpMIXED3FGL J0312.7-2222@j‹†DR?hÀL×Y‰ßsÀ:h©ÒÌÁÀ;µÙÅٔ?겸›VL@ ¯Õñ
Ê?ùÿ¤ÐÚ?îR'äɘ»¿Û¯ÈqÀ®ÿ?ÖáëxşÿÖÃò™Ì*¢UNASNone@·Ÿ$ÝPowerLawnone?ïø!Þ2a?Kxû/Å~Ú?Ox‡''í?Kxû/Å~Ú?ï¾Ò+d}?'n`¶Ò??€Ku+¨Ð?'n`¶Ò??ï¢K	qKz?ƒù£™É|?‡m=™^Mx?ƒù£™É|?ï°
ƒf§?qc³ï"?ƒú}[¶º0?qc³ï"?ïöf«7"?QHÿìŒN?S3èÍLç?QHÿìŒN?îÉ3IÐÐà?´Ú1"×?£lËcÎÙ?´Ú1"×?ïKŠÓ‹¶`?'¹Aˆ>0?–Ž¥ŒÑf
?'¹Aˆ>0?ïW›iÊÁ?…s·þ<9?Œ*Îß¿?…s·þ<9AGN3FGL J0312.7+2011@dP¿Ž`€À?›Gb• ŽÀ:$o±hÃ8À;—¨=¡K?¿ÛÃ5#Î;b@XšJïg?û_¿^Õ¿ïI;Ø?áßN¼sÒ¿ÌЊqˆƒr¿ÓÔÃáÁ¦~UNASNone@»Æp£×
PowerLawnone?ïÿ|TÞ?ñ½÷"kÙ?u'¡b9?ñ½÷"kÙ?ïÑEíÊô0?ŒPçLu'Œ?w]ú9"d?ŒPçLu'Œ?ïê­×"&?UýI["†?eíRM‡¡º?UýI["†?ïþ1€¢õ?ÓË×.Œ)?,çù²¥ö?ÓË×.Œ)?ïÿcˆ™Ó?
ÄÐ*°Nm?ŽåZ£ó¹?
ÄÐ*°Nm?ï<¾pØI?¯ì¥b|6?˜h1ëÖ"?¯ì¥b|6?ïê,¡ÑÞ?g®Õ4Ê?eÓþD?g®Õ4Ê?ïõ=6õ¾?K Ìi8Y?U…'¿y?K Ìi8YAGN3FGL J0322.5-3721@n¾"åÞÀLY@_k bÀ9õM–ÃüÀ;ÞGòù?å>k¤Ø€Ï@.:âT@™* :8?Øj*ÊȪm¿âÓ¶Gnj>¿åß5C}n¿é'l8YÛ
UNASNone@ý¾vÈ´9PowerLawnone?ïì®vöV‰?dãCmPX?cQ‰B¹?dãCmPX?ï•ïé1‡b?"±ëY†­?Š"¬¾ï§?"±ëY†­?ï;¸ÓE·Å?Ž–tÁµüÙ?˜ˆå'!b?Ž–tÁµüÙ?îÀϓ{?ˆ²C-ۑ?®Óóì_,?ˆ²C-ۑ?ï€/Hdj?'ÿÎûÒÔ?ù´#˜'?'ÿÎûÒÔ?ìrà^hÚÏ?¾k!Ùf¹?¼hý¹)Š?¾k!Ùf¹?í4ü:ðä&?¦lDó`E¡?¶X*0¬Ð?¦lDó`E¡?äRG©"?±x*H:ò¾?×Ó[p­Ö×?±x*H:ò¾AGN3FGL J0323.7-6038@qB¼£n/ÀGç4.ÛµžÀ:|#²Œ¯¦À;àÖìá?K¿ûð ;´·@j‰9Ðf@"È߂\¿åy3Ѥß¿ì¬\`ÂÒ<¿ DÏI'¿ïÿ·`²zðUNASNone@'Âlô!PowerLawnone?ïþrwÒۖ?.Œ©C?(ØŽ¶?.Œ©C?ï֊U®Þ$?Š	v?tºÕbáæ?Š	v?ïY™øÛ?Š<¾_<I´?"ÌÀûlÏ4?Š<¾_<I´?ïÿë+ÌPj>ãÌf?‹0•>äÔå+åƒ>ãÌf?‹0•?ïÿ"qós'?ï"BïÖ?#Š	]1,?ï"BïÖ?ïJò7sx?¯¨´Aq?–¡¹æý?¯¨´Aq?ï8£?é,²?•þ˖y¦ ?˜ë˜"›µ?•þ˖y¦ ?ïÿ÷ú^<?"׸Wc¸? ûÎÇ´?"׸Wc¸AGN3FGL J0324.5-1315@hï?»×²ÀIÖf¡ÉÀ:R\±±¾TÀ;Ó&
UÄXÀ	rö퇭^@
†Nž)Ì@,è…Ç*¿âÁEiãì¿î¿æ¬¿3?kîb†£k׿ïÿ¹±3ŒUNASNone@àv_Ø­¬PowerLawnone?ïþ+Æú7?/ÙÆÍAhô?-C'+zµH?/ÙÆÍAhô?ïÙ·(B5Ò?‡øI\¨=?s$kÄ#0?‡øI\¨=?îïÆ®Çöq?''¼¾æ?¡•ÈÊø?''¼¾æ?ïÿÿ}å6>¢ìÐ.'ý>]yœ¿>¢ìÐ.'ý?ïÿWAï9?"L¼;R?ñÚ†_?"L¼;R?ï]A~qíP?¬Ø¨(KÐB?"WÐ*ã?¬Ø¨(KÐB?îÐEI­•q?›ÕZr¹Ç<?¢û«a·ï?›ÕZr¹Ç<?ïÿõ
ÙwÖ>å
˜æJA>Õêcf¸B>å
˜æJAAGN3FGL J0327.4+5828c@aÄí(Œç?øÝÈgã>(À9vG…À;ûXÑRn?ï0=÷(ã@Âg
€F6@•À8–¿ÙÑiüÀQâ¿å®üd¿ó ¿ì="ßEu¿æÿBpÆoUNASNone@"8ï4Ö¡bPowerLawnone!?ïŒÁû=2?´h7*qj<?ŒÏDÿ‡Œ?´h7*qj<?펶̰G[?´"éä'é?³ŠI™¡Þ)?´"éä'é?îb­y Tõ?œ¹X=é "?©Õ(eÉ·?œ¹X=é "?ëë=|Èd?–áƎW6Â?ÀSòÞq?–áƎW6Â?ì†<ØM‰v?¼Ç}§(?»Î="´R?¼Ç}§(?ÜÄ%Ö ­?Ïí˜Ð­Y?áí¯©??Ïí˜Ð­Y?çގORgp?¸^$l~«?ÐBãa[1!?¸^$l~«?Ø=  ÖO?·ÃÙµ¶—?ãáoô¯"Ù?·ÃÙµ¶—MIXED3FGL J0330.6+0437@fp¯%;ÀD]9–úƒÀ9º~¸lÃxÀ;'ØåßÃJ?ìJ	
šÈ@|Õ@8Õ@ä`RP/¿Ï¹2À`qŸ¿äÖƄDƒú¿Û[kP…ÿ^¿ïÿðH°{'UNASNone@"'ùÀëíúPowerLawnone?î(Ø ñp?´ÕO˜ ?­~b}ðé?´ÕO˜ ?ïd›9p¨Î?'ãm#ú%?"l˜Ë®>?'ãm#ú%?ë!¿~–Å?ª1†ãCÃ?ÁÃy¤ì?ª1†ãCÃ?헤]%?Q¶Y'x!?³BßFÎ¥Ó?Q¶Y'x!?íì՘?ºÀJªÀÚ?· ˜‰ ¿?ºÀJªÀÚ?ìv«"á‰ü?»óÓ)Ð¦?¼J¦èó°"?»óÓ)Ð¦?ä_Í¡ô?½§™ÙÒ¼?×AÐeļ?½§™ÙÒ¼?æe´p?P?¶†6[‹à×?Ó4—ہ_?¶†6[‹à×AGN3FGL J0332.4+4644@b¯a¦
EcÀª	EùßUÀ9®?uŒÀ;k|Ìy1?í[µ‹Ás@
c?aì@À}àU•´¿á±²-þÛ¿êŒtª7e¿æËirµT5¿æ»Kô
˜UNASNone@‡/^ÈtPowerLawnone?ïÈMR)~»?"çÓA
Äí?{ÙW	}2€?"çÓA
Äí?ëߢ«Џ?À"Žw…?ÀuSœ½Ä?À"Žw…?îúVN¸—?"+'+˅±? ^š8Ž?"+'+˅±?ë4kyö'?šE—»}W	?Ã.R%»¦?šE—»}W	?îYhÊwe›?²@`aLr¶?ªisW­¿U?²@`aLr¶?ÓZùÂ	‹€?΄NǃÀ?æRƒû:@?΄NǃÀ?ë'›#ÿ°ò?±ÌkqˆÆr?Ãa"p<8?±ÌkqˆÆr?Õ#°}z˜ç?´Óà,õ?ån'ÁB³Œ?´Óà,õMIXED3FGL J0333.6+0233@fÆÝ/Ÿ¾ÀDwŽ`€sÀ:;à5_]^À;»*‰@†¿ðÏpˆ©1g@
+Ž
{"@'vŸït¿ÜÏ?ѯ¾'¿æ~øù?¿ÇÝ0r9¿èæßé<͙UNASNone@¤vÎ!–R½PowerLawnone?ïþ¾ÍcS??"I…q(?$-£õ¢D?"I…q(?ïÔºûF»Y?Œ
¡Òmã˜?u¢'v¿[i?Œ
¡Òmã˜?ïÙ¾]¯o?m¢Îv›ê?sr íUo?m¢Îv›ê?ïþßCœâÏ?‡»X?"Â@y'?‡»X?ïþuZ0^?*	J–¿tŽ?'(­ÕaâÎ?*	J–¿tŽ?ïKÅðÜîÐ?¯¨jR:Q¹?–‡A݂î?¯¨jR:Q¹?ï¯IKDï@?"Ðk‹ëæU?"-­#mz"?"Ðk‹ëæU?ïó÷ÎO¦(?Tt©zf¹?Xcf3%?Tt©zf¹AGN3FGL J0340.4-2423@kQÃóà7ÀJÆ)ñkÀ:œ+Àx*´À;ð|_Ìï1?À¤7F,#@
'Ù@µ/ßì5¿årekÐĺ¿Ú0—–£ß²¿äÀ9EñÑ¿¿áð™#ì³UNASNone@¤{_b¶®}PowerLawnone?ïý|6K/m?BU+œ"\?4N'))²?BU+œ"\?ïËV¹˜?ŒœÚì &Ñ?zvÿNsèD?ŒœÚì &Ñ?ï»Ó˜÷eÛ?w¿}2aN?Ë…(?w¿}2aN?ïPYÑ?og9‡L›R?ˆ«é¹}ËÄ?og9‡L›R?ïúCá÷?H]Zä2»?GŽð3JÈÓ?H]Zä2»?îMÖåªiK?´Œ3¾>+Ä?«"'¤}"W?´Œ3¾>+Ä?ïz
vë2­?ŠÅ–>ôœ?¾±r@_?ŠÅ–>ôœ?ê£é£5?±þv¢z'
?Åp[ÿýs*?±þv¢z'
AGN3FGL J0342.3+3148c@d
â'@·€À2a"D¿À92»K›	À;,äd™?íϣԅþ²@ôÑø/Ò@5F@V1e?ïã–>§×¿çA½¦ˆÉ¿ç*éy<;¿åGÅ	›‰UNASNone@˜•¥`A‰7PowerLawnone0?ï¦1âPB?'J7ÂË'l?†}3ƒüS—?'J7ÂË'l?î¢BÚ	7?¦º5ã•$æ?¥ÛÒ]·>'?¦º5ã•$æ?îEèÇÕG?Ÿ>ŽW²t?«¡sÒ´‹?Ÿ>ŽW²t?ìÐdÀZ3ä?—ž©Aåû?¹|Ùûv'à?—ž©Aåû?íK<QÈ}:?»H­Ì_N?µ¦pH/?»H­Ì_N?çou@žÖš?Êb©oœèP?Ñ!~ÂRË?Êb©oœèP?èkõêRn¸?¹6abáñ?ÎP(V¶E!?¹6abáñ?âŽT
–?¹¾›Aö€·?ÛýÔãWäÕ?¹¾›Aö€·AGN3FGL J0342.8+1321@eƇçÀnÀ?÷\9¼º0À:z¦ª#T™À;¥ôæò?ä0ÈCiûá@
LØÑÞ?þ‹¾_K¿ò?¯&ˆÀXu7¿Ë
ùЈ¿á®ä^ä¼Ù¿ÞO•vk¹"UNASNone@²jÞi­CPowerLawnone?ïþOñÚÎB?.9Îý,|½?+àÝF]Û?.9Îý,|½?ﺥlØè±?,_z&O?V¤ÄFs³?,_z&O?ïÑTÕU˜Ÿ?s‰.o¢?wU•Pd<…?s‰.o¢?ïxAH¬ä?oŒçUux?÷Ðɛh?oŒçUux?ïúìI·%"?Dwÿw†wá?DNØ=nÉ?Dwÿw†wá?îTæÉùé?µ‡g(]`;?ª±"\#þs?µ‡g(]`;?ï{L	©?‹ê¶ý¨?–~ÔhÄÝ?‹ê¶ý¨?쐂:±š?£3ìŠ8?»{î/js3?£3ìŠ8AGN3FGL J0348.1+4431@c!Ù©T"ÀD=F²lÀ:;ÔÂeÀ;n=)HÏ?ºŽ›t÷4@-}ns%@5G zô¾¿×¥Á'~iµ¿çÑÚ?üð+¿èduØÊ1¿ÔDRû$¤UNASNone@˜Em(ŒçPowerLawnone?ï䂪®ƒ¥?—øÉÚóä»?k}U¢"ñ?—øÉÚóä»?ï«ìð?'ͯ	"2¿?…:ÿuåŒ?'ͯ	"2¿?îï'{L°?—.P»ÓW?¡
ˆFé|?—.P»ÓW?ïÑ8Hé?bšÖɐƒL?w@cÜïà?bšÖɐƒL?îîÔ×æ¹æ?¨01¶œT?¡²~$Ş?¨01¶œT?ìõ7cˆTg?¾*Û~tã?¸VDâáuÌ?¾*Û~tã?ì)B¼ñ–
?²¿í›mg?¾µêsO"?²¿í›mg?ìÉÄ¥òÿx?°'"c?¹±ÚÐhC?°'"cAGN3FGL J0348.4+6039@aßî$5in@‰Ð~25À:2‰'
ÙÝÀ;± žÛù¿ÓLI¦@
^'í'úÇ?þ4A%9J?ïþ"¯OÖ¿ëÞðQJö¿×<•ì»Ö¿…8…âÀo•UNASNone@¼î–E¡ÊÁPowerLawnone?ïÿ`È96¥?Aêi¡ä?æÿ¼ÉBò?Aêi¡ä?ïÀðK¾*¯?"ò®ã̦?‡Ú=Ç`z?"ò®ã̦?ïÎð˜PeÀ?{WÑ.Mž®?x‡³Ó­—Í?{WÑ.Mž®?ïþê,óÂÊ?ÝRØÅ?!]4f9·?ÝRØÅ?ïþ¸(H?)½}ú'?$}~?6t?)½}ú'?îÀNåžÞ[?³¾®$`ʀ?£û¦îU?³¾®$`ʀ?ïЎ""ö
?xŒ=!àÛ¼?w¸¾"¢¬?xŒ=!àÛ¼?ïøRS¬Fè?I)«VE?N¶±ü°?I)«VEAGN3FGL J0351.0-2816@l,@N¤©ÀI:žË1ÂÀ:½4Ùü`8À<ßÇ{T4¿æÛL@
1S1€U¦@WL_ª	©?ëB³ÔáÌ¿ÜÎÊÕô
K¿ç-@µ‰˜¿Íp³G%ëUNASNone@¥èšáG®PowerLawnone?ïýŸ¡«¢?1" '' ?3ò¦•{;?1" '' ?ïÕBûø?Œ;=ÌFó?u^ùœÐæü?Œ;=ÌFó?ïšíŒ_õ3?}lAu)óz?‰Dœîáë/?}lAu)óz?ïþÕ(Yæ?ä8qD?"®+"]?ä8qD?ïû‰Îñ+?@ñ¿9óy?AØÈ z®?@ñ¿9óy?ïJ3ÎAIª?¯×K¼"!ì?–¹†4g.Æ?¯×K¼"!ì?ï=† Û?•ÖS·¡½6?ŸØO=Ô°?•ÖS·¡½6?ïí0<'?a*·=3\?bÏúó‰v¢?a*·=3\AGN3FGL J0351.4-3248@m"ßÎ1QÀIs,B»fÀ:eZJÏ1+À;õ¯OäCâ¿Úp6Úîµ@JÌõfžð@`g "I׿è%¯ó´Sj¿ç=‡ëlm¿æc¨]¤n¿ïÿê†úŽ/UNASNone@{˜=Ùb·PowerLawnone?ïí4iû,˜? <&>0¦â?b˕æ–Ø`? <&>0¦â?ïÌ7‹)
Þ?Œ_ð'0J¿?yä:P­U?Œ_ð'0J¿?î ³Þᙰ?"Ãþ]m¸M?¥ôÂzþ?"Ãþ]m¸M?﩯Ø0"Y?pÅ1Ÿu«È?…"	þ)½É?pÅ1Ÿu«È?ïú–¢öÝ?P£|p
Îi?E§¨ÛÜC®?P£|p
Îi?î="7ï›?·ï y?¬-܌QjR?·ï y?Û+	n?™-kþ=Α?¦UrJ»´"?™-kþ=Α?钱Þ^ð{?¶çG4b?ɵ8†">?¶çG4bAGN3FGL J0359.7+7649@` Âø7´¢@1ÐWÙÛ©À:¥ID°FÀ;þb°Ï@E¿ÜôP‰Û5›@ñvæ;^@Sù`(´ª¿í,#³Iª)?¨,ôÝ¿ä8B¿è‰¸Ÿˆ	éUNASNone@¢Ãñ[W>«PowerLawnone?ïþ·<º?%œcê
>Ó?(‰é;<±?%œcê
>Ó?ïÕfUcMœ?ƒm˜æ""º?uLÕRx¹ø?ƒm˜æ""º?ïÕb"'"°?vp¤z?®Ž?uN£ñ?vp¤z?®Ž?ïùûÌ(J?4/âi>Ïs?HÏj]ýg?4/âi>Ïs?ïý@ŒÚeß?3ÓÊ©Úà?5û—ÛD6Ö?3ÓÊ©Úà?ïàÞ7êc?±
µ~ÿâ?ŸCä0k­£?±
µ~ÿâ?õñ'Ü?‰å¤>v"ë?‰€+í?‰å¤>v"ë?ï­
iA"|?z>p6÷sw?"¼¥¶~ï?z>p6÷swAGN3FGL J0401.0-5359@p'4'¾‹ÁÀG'.œË}AÀ:ÚºÊkÉ}À<:L,(}?âׁα¾@Ý"bô@ɑmä	¿ã8Ûn®¼õ¿è¤ÐÌX*0¿æŒVöq€?ÒPJ¹?YæUNASNone@¡ˆ$ÝPowerLawnone?ïúq8…
I?X‡Ó>›?F;Yš¯Ë?X‡Ó>›?ïÊ)ô'…ö?ÝƒQ¤O?zë®}ôÓ?ÝƒQ¤O?ïs Nr1~?‹µMÂ:(™?'‹ö3qž2?‹µMÂ:(™?ïè5Nt	ñ?\n¥ØP?gʱjùό?\n¥ØP?ïï?ËÇê?lÍ˗óó?`À4$Ø!?lÍ˗óó?î7XMì>z?¸]ÏÐù‡_?¬Š{ `1i?¸]ÏÐù‡_?îTÚi\SØ? ?Pv´?ª²Yeï?‹? ?Pv´?î}R@"š¬?§Å(ë;	Ý?¨*Ûö¶U<?§Å(ë;	ÝAGN3FGL J0402.7+2616@døP›ùÆ*À3"{՝VÀ9Ó÷Ò4ÛÀ;'‰¬¼Œ
?—½Iëêý@\ut cM@.Ðg¤T¿èU‹ûÝm¿él"©¼¿å'Ó¾¬¿ïþ[híxUNASNone@z›k¹Œ~(PowerLawnone?ï÷ÌåÌM ?PŽ"NÕÂ<?Pf4ëV¿?PŽ"NÕÂ<?Kçq`7?A6"M_?€Õ(p>?A6"M_?ïg+Aï†?I#<̋H?"—Ç6©Ã?I#<̋H?ï¦<C
'?iUy:õ»?†pïC~¶¾?iUy:õ»?ïçüpð?l¿€S,ç?hÊ~L?l¿€S,ç?î a€;W?´*óL•W?­ùïêÿˆ?´*óL•W?îݤ__$í?˜×…ª§È?¢%ºÂ.0?˜×…ª§È?ëë0+°¡¸?§E¸Á´2?ÀS?Q=y!?§E¸Á´2AGN3FGL J0412.0+0229@g³ÞÊl À@¬e"¯OÀ:
㎰1ŒÀ;'Á.32¿'-Q^·ÿ@V±Ÿõ©@0oß`ù¿ç	mý^¿àŸÁ¿ìšr
±¿Ë×2®uk3UNASNone@«ÜÆ?PowerLawnone?ïüa)»æ?Lã݉;ñ¹?<÷¤Å?Lã݉;ñ¹?ïÒ7Öí`?ŒDçq°õÀ?vä©
·š?ŒDçq°õÀ?ï¢ÎkÞJy?~µõXÓÉö?‡Le›mÀ?~µõXÓÉö?ïüTEÁD?+O-m…?=]Ó2‡èz?+O-m…?ïá&Ù]©Ô?uœpޗT?nÙ&Æ?uœpޗT?ï8  ›Ø?¯ãÒ^Äø?˜ûüœ!?¯ãÒ^Äø?îyJ¥{á3? '—ÿ¹?¨kU¦ŠÑ? '—ÿ¹?ïÊè×¢ò;?tBæC;J ?z‹"êzo?tBæC;J AGN3FGL J0414.9-0840@i;0©7 ÀCMs\.ËÀ:4õIØqÀ;Ï$Ù¸¿æ{ÄА7@ÚAP'Ny@:³ɹȿåªñ)gFO¿å¼;÷k˚¿áû&'ÕŸ¿ïÿ½¶¥UNASNone@õ´!-wPowerLawnone?ïþ
2™?%ˆˆÚùK?&þ¢
Ì°?%ˆˆÚùK?ïӅ ™[9?ŒB–
Úx?v=oÂp«v?ŒB–
Úx?ïyQ»ú?~Až?Õܘ´?~Až?ïúé:k¶²?3¤_Må?D[Âñߗ?3¤_Må?ïþ½ßÞi?+½¶ã#3?$"«ä–Ò?+½¶ã#3?ï@¡t?¯–÷åÀ"Í?—ì];íx?¯–÷åÀ"Í?îË?iªò?›«¥åôc?£L	gä"	?›«¥åôc?ï¶Åu¯Hq?w@
- \?'N¢¾G²?w@
- \AGN3FGL J0415.7-4351@o#zcslßÀFý<£}šÀ9þ¥é34áÀ;ø½$¹í?Ûytß꥕@
T—'hÐ@݉ÿ󕹿àe¸Û[ä¿çŒÁ!¦v¿í.	öV'¿³9¼k—UNASNone@'•`Þ҈ÎPowerLawnone?ï¹j@‡ý?´G25à¡;?¸¥}Dz·?´G25à¡;?ïËezicØ?Œù±ç&?zMB­Áp+?Œù±ç&?ï9l´D{ì?'°ø"+`e?˜ÒirI"?'°ø"+`e?ïÂD‹äê?n[&£Ó?~ûÝ»mc
?n[&£Ó?ïÀSäûå?SÞ!Ô~,?Ö
"›^'?SÞ!Ô~,?î-víêv"?¶ØÅÕ-?­('#ìRÖ?¶ØÅÕ-?ìÎúL,?¬à9Â훑?¹È.`?¬à9Â훑?ëeéÅ<Eè?ºÁ'›ü?ÂhXëèa?ºÁ'›üAGN3FGL J0418.2+3412@dzxl"hÀ'ǟfb5À9ÿ9¶ÚóÀ;…vfŽªR?Æîê['Ê@
íyøêb	@úg–
H¿â:|l{íü¿ëÞ0Ss´G¿§¦¹—Úµj¿ïÿù½p¹QUNASNone@'Ê€4mÅÖPowerLawnone?ïÛ¢9jÅ?¥éššÂÛÕ?r.ãX¯…?¥éššÂÛÕ?ï¨J?ý??'dX*t®å?…íp+B@E?'dX*t®å?íøÑWËîÖ? ®–²²ºë?°9u@V®Ï? ®–²²ºë?ï¦bã¶/?r m·×/ò?†y§5ähu?r m·×/ò?ïê)Ž®å?Än4¶?eÖqÄ?Än4¶?ífàDlÛ?»;² Q?´ÈýÛ²,?»;² Q?ìøêý0å?©0³àtÇ?¸8¨T¾?©0³àtÇ?îbÇå ?ª) qÖÛ9?¯ÎÙÑÉßþ?ª) qÖÛ9AGN3FGL J0419.1+6636@a±+Iº@'#póˆ"À8åbøÜ°À;e¤ëàŽ?ê§cۋpP@(ÛèH©<@~@Jª¿âÎð´f,¿áލf_A¿ã°ŠÕd)¿íþƒŽ¯UNASNone@_wškP±PowerLawnone?åÖÕ_|?Ç҈\Ÿ,?ÔRUÕAþ?Ç҈\Ÿ,?éôž–"½£?æzTÒ6»?È-…¥­	t?æzTÒ6»?éIuSáuô?°<²ð¥"?ÊÚ*°z(2?°<²ð¥"?èâIûe€?¢j• ë¼_?ϼvØiÿ?¢j• ë¼_?Ðæ_N³Ûÿ?ÅÎ2a•àì?çŒÐX¦?ÅÎ2a•àì?ÙbYûý?Ъý'×!?ãtÎòÓ?Ъý'×!?ÙOçïhH?¾+&þ+j?ãXKþÜ?¾+&þ+j?Ë7´è?¦B—3 ±à?é2؅ù»?¦B—3 ±àMIXED3FGL J0420.4+1448@f|Rç-¡#À87:G#«À9µy1DEªÀ;TÍè«P?êûˆnp@µÇ'`@î¿ÙtP¿âÄMA§?J¿îŸ<=?¿ï"¶|d´?äaU¬žÔUNASNone@rÕï½'=\PowerLawnone?ïòX‰ÑFü?j<Ò5šÖ*?[Nëú}GÉ?j<Ò5šÖ*?ïıÃ1¥?»ô'þ£i?}§s"Ùi?»ô'þ£i?ïW¸Óñ"<?"b?•刮°o?"b?ïôûeD0?S'§¾eû?V	5db"?S'§¾eû?ïʾ.›Á4?…ÙN?³?z è©àVG?…ÙN?³?îu@µìzV?¶=•ªÕ3×?¨«ô¤§öœ?¶=•ªÕ3×?íŒÉ¥â
?£;ùš$Ú?³™²Ò§a–?£;ùš$Ú?ïÓ#º*š?¦>n½²Y'?œÅ›ŠrzÀ?¦>n½²Y'AGN3FGL J0420.4-6013@pò~|áœÀDäcÇOµÀ:—Ì9ÿÖÀ;åï3ÿáÍÀqãá'Tý@
š%ۆÎç?ý†Jßø"¼¿ìCÉ»A×]¿Ä|øƒßÈþ¿ÞM±Ôx蟿ÔkËCØUNASNone@®Ùó&Á¾PowerLawnone?ïÿÿû±?£uÊùYô?€&Wž?£uÊùYô?ï×eL_ÿð?ˆ@Ayø?tMY팫å?ˆ@Ayø?ïä知¼?eՔ ü.x?k`ná§S?eՔ ü.x?ïÿÿ¬?…ô>Œæ-Ԃ®>"õŠÚ£>Œæ-Ԃ®?ïþ¨¬Çc? ³
œ*M?%ÑíµçÁ? ³
œ*M?ïQ¯8x}¦?®æWÒË£?•Êê>?®æWÒË£?ïàcP˜…?r#•xþ¨?oœ¯-Á‹?r#•xþ¨?ïÿô=Ãɳ>á´6n2P«>ׄ1®©>á´6n2P«AGN3FGL J0420.6-3742@n	E¶ÃvÀF˜#πÜÀ9[x̚xÀ;£Š:?Ón±Ê¤@凖ŒÉÒ@®m@ .3¿å?Æ ¿ã>ÍI¼ä¿ç†ÍmËNa¿âäӏðµUNASNone@'u
Ú¹õZPowerLawnone?ïû­@H"6?Glv)Lá?AJþBŒ?Glv)Lá?ïÍçö¸Z?Œ"1í&Î:?y§ ï#?Œ"1í&Î:?ï¸l½ÿ'?x£~ÝD+?ø$Á	Ýë?x£~ÝD+?|qÿæn?bÈã÷ÊF?€˜ã‡='X?bÈã÷ÊF?ïØáºÅŽ?y~.GPÍ~?sùDùP±?y~.GPÍ~?îÞºÞòƒ?±´?¢^B×Ð?±´?î–qÑ©€l?Ÿ˜aB?¦˜âáø]=?Ÿ˜aB?ìüH	øù?¢5èóˆž+?¸¿¶<Q:?¢5èóˆž+AGN3FGL J0421.6+1950@eýR½<6À4¿ÉGNÏÀ9œTŽ†@À;]¹û8ðâ?ãø­âb@Ðf{Š
@¥ã€B…Œ¿ÙæÒ1¿æ}ô}s{Ö¿âö@O6°'¿ì–­™*ÞÑUNASNone@'yrþÅm]PowerLawnone?ïÂ¥n¹ñÿ?…0Vá˜sÅ?~­H½Óô€?…0Vá˜sÅ?ïlõ¸´è?"'|tÊÿ?'a]ãÁù
?"'|tÊÿ?íË°s‹ú? ;áÕ
?±¢|eWýÖ? ;áÕ
?îM.åyJ?ƒW"Ú?®‹-¶j?ƒW"Ú?î`µ>æV?¬ÔÀÃw?©ô®)}å¥?¬ÔÀÃw?ê'?qR?ě趞?ǽ÷;ª·?ě趞?ë&!¬št­?­j2½éÑ?ÃgyM–-K?­j2½éÑ?ä.ìWŠ3(?®EHåp3y?×¢'P뙰?®EHåp3yAGN3FGL J0423.5+5442@bϕBC@åœÝøªÀ9ü*ˆjÀ:'Ýr6~A¿±-ä?GM"@§ÃÓÔÔ@™€D3¿ãº¥¹ëý¿ìî­…M¡¿Ñ8Áïñay¿ê\ôïøîUNASNone@d—Ûô‡ýPowerLawnone?ï)â<Àæ?°?¸ÊU\?šÃ¸vàyU?°?¸ÊU\?ï¾H@œ¹p?A62oç?€mïäØEø?A62oç?ìyNþYÀ?«^½"N?¼5À
1þ?«^½"N?ï÷¤Xܲj?=²PÕD'o?P·N–R·?=²PÕD'o?ï@Ž«Ýq"?¢åIĝ"?—î*"Q͗?¢åIĝ"?îŒè!Ö®<?´öºæ¯ó?§1}â•C?´öºæ¯ó?ëŠä^}¨'?­sÜ¿µÂW?ÁÔn†	]¼?­sÜ¿µÂW?ïכŽLšŸ?iñ¹€;½?t28¹f\æ?iñ¹€;½AGN3FGL J0425.8+5600@b¸"t¼j@d‰Ø[À9ƒ!
–ÁxÀ;
¤$7îÀþü¯ég7@=ïN×Ô@Çç^j¿çü(ˆÆsÓ¿éäÅ©Re¿åa9Uâ	Ë¿ÇýºDMÒUNASNone@Ÿú)Çy§PowerLawnone?ïû¬1)vO?F^W_î¹e?AO;N›HÝ?F^W_î¹e?ïÉÅ: &*?Œ;à&é³?{cú.â?Œ;à&é³?ïz÷lý^?‹[ó%*B?¡x—Z>?‹[ó%*B?ïÿÿHíQ>›zX=ÚP>–ÞÀ½s >›zX=ÚP?ïäOz6[?qn6"¾ŸØ?k°ýb
µ¤?qn6"¾ŸØ?îêìMx.?±Á5b¢‡?¡Q>
L–#?±Á5b¢‡?íÓ®	?¦ÒñzóU?±g!¿š?¦ÒñzóU?ïÿê+,~Ž>î‡èû¸k>åÔÃF+Ÿ*>î‡èû¸kAGN3FGL J0426.3+3510@dœP	,ÏlÀ#P—ÈAîÀ9¿Îí8}À;.6Dÿä?ë+ܱ`#›@À;#°@èÏßüª`?ÄE¤—­¿èäKGbPh¿äE"‰£ñü¿ïÿô_
ÄUNASNone@'ë8ï4×PowerLawnone?ì›?¢
	!?Â!LÖÈN8?»&ﯶù?Â!LÖÈN8?ç-/$u?ÆÝýÁ?Ñ¥ÇÇ¡·?ÆÝýÁ?é—CÒ×l¨?¯Ýa³(€?É¢ð´¢Ma?¯Ýa³(€?çø\Œa¼w?£HŒm®{ ?ÐFç<‡?£HŒm®{ ?êYˆ"‰þØ?ÉÌ9g]dé?ƙßuØ ?ÉÌ9g]dé?ÍDͼƒJð?ÉA–DÇÓ?è®Ìß-D?ÉA–DÇÓ?ä;æÁH<ã?»åšIÌ?׈2}o†:?»åšIÌ?ÏD¯‹¸Y?¬†Ç!?ª`?è.Ôøj?¬†Ç!?ª`MIXED3FGL J0427.9-6704@qr(õ\ÀCE±cºº|À9cGK,GÀ;Óêçj¿ÜùüP¸@
‹ÝT@¨`ÿŸ2
¿ãõ趧
_¿çt>!½ƒÈ¿åXbü"RÇ¿å\{&kUNASNone@"£Që…¸PowerLawnone?ïø#às·?W‹ÉåŸ&?O÷o{AÆÀ?W‹ÉåŸ&?ïÎò ?\Z°?xûÿ™Ã€?\Z°?ïxÿ±.>_?†y²ëè*?à	ÕÊ?†y²ëè*?ïà劫6œ?]3ãÖ­b?ou'$;U?]3ãÖ­b?ïáÏLDI?rq€'µ½?n0èqÃ7µ?rq€'µ½?îé°>»kj?°Å¥^pd?¡dü%0Z?°Å¥^pd?î,ׁ†¨P?¡"Ámj‰?­2‡èqaû?¡"Ámj‰?íYQ>zÓË?§¤â¿P®?µ5v—U+?§¤â¿P®AGN3FGL J0429.8+3611c@d"ãû½{ À ނ/ðˆ"À9vygÊêÀ;õÊ?ìms†"
<@
¼¹"EŸ@üŸÀdµ¿ÕË룿çå#üg!Ö¿áÎ+uéU¿ïÿÖµdUNASNone@'â²ÊW§‡PowerLawnone8?ì̬ʊ
œ?¿ˆæ¿£TÀ?¹š™«¯""?¿ˆæ¿£TÀ?éw¿·?Âú&ˆó?Ë÷ö!Á#?Âú&ˆó?éÏïmób?®ëSt"?ÈÀBK2y?®ëSt"?èÌ˜"¶Ü? œBªS.?ÌÏ͝­$'? œBªS.?å´+W¿?Ðdþô߇Ý?ԗÕ©P'?Ðdþô߇Ý?ÐDÌ4y?ÊF®e-¬6?çݙþeÃv?ÊF®e-¬6?á™Bzè˜I?»÷¯ÆÎþM?ÜÍ{
.Ïn?»÷¯ÆÎþM?҄½^ų(?±º¹¸'o?潡P&l?±º¹¸'oMIXED3FGL J0430.1-3103@lìÞÊl ÀED¤Ò²ÀÀ:°+Xs^œÀ<
Å󔷳?çß™3©a@LzNP?ÿ‰ÀGƒL?ïý-óáÂ0¿äéö[ïó¿Ë:B†M[¿í€.ž*UNASNone@¤Få¡ÊÀƒPowerLawnone?ïÊDbÁ§f?|Þ#NË'y?zÝάê¼ô?|Þ#NË'y?ïyµd6œ…?"F7"8S%?ÉSy,oR?"F7"8S%?ëǶ4ÚÓ ?¨…¸—³?Àá',"³?¨…¸—³?îOÏ	#Px?z‰T÷?«mÊø{?z‰T÷?ï¸IÀheo?…b.­ÄG8?íéV@5?…b.­ÄG8?í,¾mè]?ºŠ30j<E?¶šd½?ºŠ30j<E?í*'§‡?¦XSÍ3Y?¶«ƒi~	J?¦XSÍ3Y?êHm-;2Â?´6 ¤?ƒÜ?ÆÞKK4÷?´6 ¤?ƒÜAGN3FGL J0432.5+0539@g¿—$tSÀ;ZÀh ÓÀ9ŠDZ¢ãÅÀ;Y»JÄIq¿ípƪÚð¸@Pèà©£@ŽÝŸ'禿åëô¿íU
:ç׿×ÞÞY‰€"¿ã"+Ù-ÆUNASNone@)©"áPowerLawnone?ïÿpØ(y?òEjØPž?äô.tÈì?òEjØPž?ïÑŠbŽ?ŒšFˆp?ws:ÒgU?ŒšFˆp?ïà3YÒ6ø?inê†ØŠ
?o̦Bf°M?inê†ØŠ
?ïÿ>–‹¼?	áŽrš?-'þ†¤Ì?	áŽrš?ïÿLý<^ß?AjöoJ?`Z}OQ‰?AjöoJ?ï=@Û<|2?¯+ iWâ‰?˜W䝗ã´?¯+ iWâ‰?麟"à2c?†s.®·ù?†76Å[a?†s.®·ù?ïøv<ƒz/?Dl£0æ?N'0ÃX.?Dl£0æAGN3FGL J0434.3-1411c@jWŒ½D¦ÀB[hœ¡‹ÖÀ9ñƒ 3ÏÀ;œ£©½Ô¿é •ìÄm@ü'ã@Íÿ|wu¿ÛÀ)˜œ2¿çÚý<´ÄÌ¿ï"ÿž'À?áv×fJUNASNone@"åuâlvPowerLawnone!?ïÿkr¿»?s;núì?' J?s;núì?ïÔg*±"r?ŒGø¶6g®?uÌj³œ^ú?ŒGø¶6g®?ï¹3˜¼W'?{;]\¨%¼?³È«{?{;]\¨%¼?ïÿøF´U™>ÍÜ~³¾YÑ>Îä7
a>ÍÜ~³¾YÑ?ïþÕʑ"?,Æت›0ˆ?"£ZQ®ÿ?,Æت›0ˆ?ïKoÒuÙ?¯ô̞"N?–œR‰Úã?¯ô̞"N?ï
es™¢?—	2Þ?ž³Q'ó&?—	2Þ?ïÿ(qŒW?$|¹Î;?ÿöi"Vƒ?$|¹Î;AGN3FGL J0437.7-7330@qá[À6ãÀA˜À½ÊÑJÀ:6`áÂ'WÀ;Ô}Qœ?Ú:¿ö@ý
WFã¿@Êß^Iâ¿ç4ãöERV¿éæ—S™/<¿¦·äüLð¿àÓ´[x	UNASNone@¤J…`A‰7PowerLawnone?ïÿwˆ2û?6!¶"|?òÜ9ÿ,?6!¶"|?ïÌ4q Ԍ?ÕqÍQöÐ?yåÇpE¦?ÕqÍQöÐ?ï#õ?e;¶aޘ?aêG' O?e;¶aޘ?ïí>	%½?Gâ«5ªA?bÁ÷¡³&?Gâ«5ªA?ïÿ"нOà?Eüútû?ËÑs³éß?Eüútû?ïZ=Z Ø?±©$M:'?ž4¸Vc³?±©$M:'?ïéyΣ¼?p]çr…¦?f†1(µ4Ž?p]çr…¦?ï¶CY­+®?v‰} Ÿ\N?'o)¤ƒHp?v‰} Ÿ\NAGN3FGL J0447.1-2540@l3E¡ÊÀƒÀBØò{²þÅÀ9û=5´ÃÀ;ÓFóÚWпâɽé…Q@
>쯖0.@ÅàŽ6¿å<Ó@Àu¸¿æTþ&¶øû¿ç;M—ý& ¿è
&S?±àUNASNone@‡íC,¥zPowerLawnone?ïü¢™â-¡?PÄð"<Þ(?:ë/7ÞtÄ?PÄð"<Þ(?ïÒ0
×ó?ŒR¬g€'?vçú«"r7?ŒR¬g€'?VÏ?K˜0˜63?‡\ªN=gÏ?K˜0˜63?ïñÈvÉ,|?Hë¡èЮ[?\oZi8Ä?Hë¡èЮ[?ïúç'
Å?I™£ÿ""Ä?Dc–«à\²?I™£ÿ""Ä?ï%ØaÍÈ?°$۝V?›]äîžÝ?°$۝V?îòÏ#ziº?–Èìr£nV? Ó
Æ¡–f?–Èìr£nV?îÁ^]i£Ä?–"L¾ú›?£ê*AªÂ?–"L¾ú›AGN3FGL J0451.6+7231@aXÓZ…‡"@1‹Ø¾r–öÀ:F–À¡E`À;Օsš+?æ"+de@
فÞç×j@5.?Ù^Ö¿ê7þ¥ü˜0¿å/–¼¿Þ0‹"iAô¿ê'/îÀ_UNASNone@ƒT…¸QìPowerLawnone?ïû¥'[?C±P8U•Ú?C‰iڊ(ô?C±P8U•Ú?ï=hså^?¡«á¶Æ?œ8RøbŒC?¡«á¶Æ?'`å@?ƒ4	#?¢9?n¥è?ƒ4	#?¢9?íÜ÷á½8Ÿ?þ¼ýڈc?±@ó`‡?þ¼ýڈc?ïëNW¦Úö?m42jµ?d±¨JÂf?m42jµ?çOˆBU?Ë»V·"?Ñ`ïÓ{×V?Ë»V·"?î|€çúƒG?\ÔO·€?¨7ñ3²?\ÔO·€?ã⤦h?¹`Ó0gr?Ø;óƶ³0?¹`Ó0grAGN3FGL J0451.7+5722@bã©æî·@ £›ˆ‡"ŸÀ9¸ÀÂÓNÇÀ;n:©I:?ÜRVMƒZW@
¿Ñ2œ_@䜿¾ÇQ¿ïµoŸf&?ÐXÞ_闿ÕÚ`:Ê£Ÿ¿àèaÓ¯•UNASNone@Œ•ùdoPowerLawnone?ïÔþ÷†#?§£»]–Ì?uÿyîµ?§£»]–Ì?ï&š ¢æ?£!3?=D¾?›,«ë¼ã1?£!3?=D¾?ï=:þèÜ?'L8wF±¶?˜X½šûz|?'L8wF±¶?îȒ€u±?ˆ°SÌ.7?¨v×ø¤í?ˆ°SÌ.7?ïÄژšô–?ˆ™ç~F/y?}'³¢·?ˆ™ç~F/y?處&\$?ʀ»ÍÝ)M?͙«foä?ʀ»ÍÝ)M?íÃ1SÆ6í?£beÜÅì?±æu`z?£beÜÅì?æö-,Í­6?¶…\ÐlgÓ?Ò¥¦d¥"?¶…\ÐlgÓAGN3FGL J0456.2-6924@q‹öy|ÄÀA¤6~ANÀ9fÁæ¯ÍÀ;ŠCV–åŠ?ôUü¬
‹@!ÓÛߺ:@vQØ7?Í6;9¥¾¿é¢<²I$¿å`î¦L–˜¿áB#hºÔ}UNASNone@…—Oß;PowerLawnone?ïTiÚlÑ?—]=€Ÿz?•rĵÕy?—]=€Ÿz?íq†²ƒ—Ç?µ´"«½	k?´sÊkãAÈ?µ´"«½	k?íÔøW? ¢‰t‹×µ?±_(;íÈÄ? ¢‰t‹×µ?ëròâúÐZ?žR¢í³Õ¹?Â44t¾˜?žR¢í³Õ¹?îJR~I~q?®ì²ÑD9?«ZØ×´ò?®ì²ÑD9?ᣱ¿‡É?Ñp…*ÄE?ܸœÞðn?Ñp…*ÄE?ë3œæ'U9?«—r½€·G?Ã1Œeº«?«—r½€·G?ÞêÍúÛd?»üBä´¨œ?àò
™'N?»üBä´¨œMIXED3FGL J0502.6+1759@fö©ûçl‹À,~$5inYÀ9¼R¯Ð<ÄÀ;@½½eP½¿øŠÖ/¢!@˜‰°B}~@TZ 4"[¿àɪÄöOä¿í¢ý††Ÿõ¿æb"9éŽW?ÒZðiÃUNASNone@ŠKÙJôðØPowerLawnone?ïþ‰9­©?C&n-ùñ?/—kçÍE^?C&n-ùñ?ïÈ«šÍ÷?Ž«P?{ª2™´_V?Ž«P?ï"WÅ'«¯?†ƒœ%fÌ?‹*Àcè?†ƒœ%fÌ?ïÿýəçr>°ûì&•ï>±²ú⇃>°ûì&•ï?ïï‰ÃÁ>?q÷Ìá?`v<}úγ?q÷Ìá?îç±N/ý?°ý"—ù¸?¡"ëHY+?°ý"—ù¸?íü:	õH?©[ÏýŒeÝ?°/´Ü<Ã?©[ÏýŒeÝ?ïÿË&Pîý?Ò_ð
z>úlԅ÷³@?Ò_ð
zAGN3FGL J0506.3-0357@i+IºÀ9{úLaØÀ:©­
åÀ;vj!
?ññüÌï²U@
sà!"M¥@W=ÿjþ?ïøñ¥8"¿â4z/"bë¿ã$–-º‰¿îL‹Ç§|UNASNone@ Ï˜üPHPowerLawnone?â6
ë_$?Î<˜Ÿýš?ۓê)÷A¸?Î<˜Ÿýš?ÍúD`¶?˵ÿbÑ?è¿A.çÓ?˵ÿbÑ?äèÀ† ÷?³5M'©bñ?Ö.~ò¾ã?³5M'©bñ?Ø3v—‡ç?¯0æsñ?ãæD´~¼?¯0æsñ?ÛÏ׃µÓ?ЕN_£B?â>%–?ЕN_£B?µ`QITÏé?À¡*É?íSõÖ¹é#?À¡*É?Óá[
±ˆ=?¼5†xïCß?æRy';â?¼5†xïCß?°²O3Ëx?—²+¥
?íé¶"Îa?—²+¥
MIXED3FGL J0506.9+0321@h¦$žDúÀ5_â'@·€À:Œý­?hÌÀ;»*VëŸ ¿ùkm´3@Eþw?üމ€Fâ=?ÐaÇnÅ?¸*Ùô,׿ßAׁ[µ¿Ý&ÇojÆóUNASNone@¶Ù‡+PowerLawnone?ïþ'ÿ.W?DDü;Ø?-€²µŸ;?DDü;Ø?ïÎàã&¢Î?
yÉj9?xŽkþ¬Ê?
yÉj9?ïÚ>pN?h嶎Ù?ràñ¼*F/?h嶎Ù?ïÿÔû*¿W>î›Æþ²I>õ'cYQê>î›Æþ²I?ïû
–I6?F&;¬¯?C£Ê¦~×?F&;¬¯?ï1㆑më?®ì óB;ì?™Ã4±z›?®ì óB;ì?ï±ÞÎúF?'f»…X˜=?ƒ¿HZWÔn?'f»…X˜=?ïüê[þÙd?9Q|…EÔg?8­qI¥ž?9Q|…EÔgAGN3FGL J0507.5-0906@j)ˆe"¯OÀ;0÷Do›™À:w©"ÉÀ;¹/š!~Ö?2ÏO§°k@S[žnH@ÀÍÆ¿à£ûiº¦¿çˆ¶xU.ä¿åÁȅÑvç¿Ø¹û{ƒPyUNASNone@
­Œ?PowerLawnone?ïþئRm>?(Ÿ_µ~óÂ?"ušÝýØ?(Ÿ_µ~óÂ?ï˶ã4ö?¶ÎÍqÒ?z$Žp>Ù?¶ÎÍqÒ?ï½yWž?vå°7±˜L?€¡¿MøLS?vå°7±˜L?ïñ4&¼ñý?D'6zá*?]—³MU	?D'6zá*?ï÷NÿZ?YL"özÊ?QÕc@[W?YL"özÊ?ï9ŒFR}?°Yp±.?øÎnžªa?°Yp±.?î'äjÇ8?£þüÕ-Ä?¦á¿‹çA}?£þüÕ-Ä?ï8Ÿhæsg?‹=Š>\Y?˜ìæ¡/?‹=Š>\YAGN3FGL J0512.0-3737@n0mÚÎîÀAˆƒ¡	ÐcÀ:¦í_‹ÎÀ;æ»:Ôe?Ér¤|‰Ð@
u>mÎå@™Kãö	?ïÚÙÔ¶êÒ¿ê+ýw˜œ¿æ
W	.Û¿×L…ϸ9˜UNASNone@¥Úg ù	lPowerLawnone?ïþ­îBñË?&€‹Ëî%?%!˾À@?&€‹Ëî%?ïÌ`=Ú?ÍE¨Ã?yϱ]ŠÉ?ÍE¨Ã?ï²Áâ±?wjôC?ƒO´§Ë¹?wjôC?ïç$ËÖš?Sé~C‡Ö,?hÛ3ñŠÎ{?Sé~C‡Ö,?ïýÊ6«žæ?8U¹AÿŠ9?1®KÒèu?8U¹AÿŠ9?ï
Ãàù?°íú+ñ³?ž\ç~Ø6Þ?°íú+ñ³?ï!ÉìüÔ?–шc?›ÆÂ[T›€?–шc?îúáµ½Â?"÷æšÐò? Qä¤.óÞ?"÷æšÐòAGN3FGL J0516.6+1012@hû¼¾bÀ/v(í_ŒÀ:cŒT6¸úÀ;yÇg2>A¿ÒÚ#ޒ®@Àà"ÍR?ÿþî_ċ¶¿ê…³tG`οâÔ¤::¿Û¬³Ì9˜Â¿À4?¤ÓUNASNone@´¨U¸QìPowerLawnone?ïÿPI·?7%
@Å?µû'Kf?7%
@Å?ïÆm`[ø?I³Ãt0?|ÉP±<!?I³Ãt0?ïãh%|Å?a:¶†Ð™T?l—þ\2Õ?a:¶†Ð™T?ïþ@PŽI?P¦eõ~?+úöiOÂò?P¦eõ~?ïüì'IÆÈ?:Ìô'Ã2+?8›î0;[r?:Ìô'Ã2+?îĝ-ÍØ?²Tð_˂û?£¶-#ÿ­ƒ?²Tð_˂û?ïʆáR8?z7Á`P®^?z¼iGGä?z7Á`P®^?ïí­+x?\#ðÐ+3Ý?bRÔü'°<?\#ðÐ+3ÝAGN3FGL J0517.1+2628c@fSµIùHVÀvvþdŽÀ93PdŒÀ;}#AM¨?އµËYÓ@@ó#x«
@=ô|ô¿âØ(š L3¿çŠK}#cª¿â‡ê©›^/¿ïÿòh´UNASNone@ˆZ‡+PowerLawnone%?BH‹? =gág?›oEP? =gág?ï²H<.Ú?¢(J£œ?œ‰¶øz$´?¢(J£œ?ìÐ~wv¦r?¤ŸÆ±åÌ?¹|B'þs?¤ŸÆ±åÌ?î9léjðÂ?‡Z2¾}°ƒ?¬i1lÀÖ?‡Z2¾}°ƒ?î¶_l;v?°¿=Μϒ?¤š	;t£?°¿=Μϒ?緈›"8m?Éʐ²jK?АîÉ»'?Éʐ²jK?éÛub ?²Žèlü²¸?Ȓ+Þw'~?²Žèlü²¸?äo!ýŁï?´(<¦o?×!¼tü#?´(<¦oAGN3FGL J0523.3-2528@l†wFˆzÀ=ӌ†‹ŸÜÀ8£¼:®Q¸À;iÉü7ôc?ðî[Ý÷A•@R$óÅ@;ÿûù5¿â‡¡1h'Ë¿àq•¥ ê¿áUôúâ¿î²"ãøõUNASNone@Õ¼¾aÏÿPowerLawnone?àØ­º§ ?Ðõ+ß#?ÞN¤Š°¿ó?Ðõ+ß#?áÅ2¢r8à?Ð0Áwë…?Üuš»Ž@?Ð0Áwë…?æ"ÄBd©x?²pâí'?ÒÖw{6­?²pâí'?á™ó‰O¡?®‰þ;Ç»È?ÜÌía¾?®‰þ;Ç»È?Îíˆë1Íê?ÊÓ/c+.¾?èDÅ3Œ†?ÊÓ/c+.¾?Í/§êLÔ?Í$ª9:£?è´;ÅlË?Í$ª9:£?Ô!‹lŽ?»wÈNQ¶?åï?:Iõ9?»wÈNQ¶?½4Éòc"?£õ¤ç"h ?ìYfÁ³œ®?£õ¤ç"h MIXED3FGL J0523.7+3328@e´×
=p¤¿÷"'àÙìÀ9;þ®Ç(À;#Ððx?ÁÛøCžu@
E¤—yƒÐ@b †ˆE¿äŒKÑaæ¿éè¸
"'r¿ë3R¼ ¾M¿â"3í~"QUNASNone@~C€ˆPœPowerLawnone?ïìêvß?v'þÏ⬌?cúpMâ¸O?v'þÏ⬌?ïÃÊ£/x?£¾ÚX«t?
LåN?£¾ÚX«t?ïæ È1?'GӆØÕL?£;ýÞÇß?'GӆØÕL?¯3ƒ?r.õšL -?‹ÔT(ìËT?r.õšL -?îäŒçœî?¤¤¹->Å?¡·?àªJ"?¤¤¹->Å?êɗñxÓ¦?Å'øÂt]?ÄÙ :±g?Å'øÂt]?ì†U¢§gì?«4"-à=?»ÍRêÄÀ ?«4"-à=?é9BtwT?¶—†³§§?˟ö."±?¶—†³§§AGN3FGL J0524.4+2839@f7…ðoiDÀ.çğסÀ9SS@ï´XÀ;5ÛNoϜ¿ñš%ȼqá@ÌwSH§d@þ[`m~¿ä ñðÞ¿à(çY.ß*¿ÝC—ñ	¿àø®Ž.'¡UNASNone@¥Ç¨Û‹¬qPowerLawnone?ïý›µŽÓÔ?+@h_SÎ?3"T(Ï>±?+@h_SÎ?ïµÕ´ýÎ"?'åßL¿ñ?'Š'°¾C³?'åßL¿ñ?ïàs—É­*?g
?ù&1l?oŒh.Åú?g
?ù&1l?ïÿ›æOÔ>ÿ›¬"G.?	KЋ…2>ÿ›¬"G.?ï÷ÌiÇç,?H,C8?Pg,
<è?H,C8?î^rjfâH?·<fRy²?ªÙXµôz?·<fRy²?ï­d¤ð9ä?†Ó‡8É[?"¦ÖÃñ†ë?†Ó‡8É[?ïúÞçg¾ç?@ò.kå?D"c;Ñè.?@ò.kåAGN3FGL J0524.5-6937@q"Ë]ÌcñÀ@jq¼Û¾À:VýŸÓo~À;šFfޏ?Öà•©Ay¿@Âԏ‡?ú"YwI8?ïíNc œê¿Ýwúã`¿à(¨dQ}?Ì@´Ê'M	UNASNone@Å(r° ÅPowerLawnone?ïþ*âÏ?*ÃUå×?-QÎÕ#c¾?*ÃUå×?ïÌø/0o?ÇÂÓ¢õ{?yƒò…ôl=?ÇÂÓ¢õ{?ïÈã%K5€?wâÙE's?{ŽmaDx?wâÙE's?ïøÀy¾n!?>òÚú²ÖÄ?Lþ¯š£z?>òÚú²ÖÄ?ïû:u"#/?CY®«õk
?C)öÆ	?CY®«õk
?ïõ9AY?±bãtåøE?aXÛD|	?±bãtåøE?ï'žM»þ?ˆÇT6å?‹i!d{?ˆÇT6å?ïÈ좢y4?wŠ{óÜ%C?{‰®¬¶9?wŠ{óÜ%CAGN3FGL J0525.2-6614@qD¾aÏþ°À@¥ÌBcQßÀ:ëíúCþÀ;¤ß³Y^@ÀÊJHùn@ ]-X@Ý<à†(?ïóšÑýä¿ß(l\ìâc¿ãѾÓS¾]¿Óâ'–¶ªUNASNone@¢²í\ú¬ÚPowerLawnone?ïÿ8hb{1?Ë-W¯?òøgÝu?Ë-W¯?ïÔÓ Eg5?Šn³‹í?u–oѝ¹³?Šn³‹í?ïÙCD<3Ò?pñJ¢è?s^]Òã??pñJ¢è?ïÿýË68>®ñ]c@Bn>±¥çÇ©I©>®ñ]c@Bn?ïÿ'º¦{ø?FÎt‰µÉ?©
¿h?FÎt‰µÉ?ïMeŸí=?®ç´Oj…â?–SMíº&Y?®ç´Oj…â?ï¾+)#Ò?¢éLû?€u5°ì¿'?¢éLû?ïÿӶ垚>ý±tÎu¨>ö$…;†XŽ>ý±tÎu¨AGN3FGL J0526.4+2247@fÛü;OagÀ¹¹"á£ôÀ9q—Å"/À:Ç)óë?Ýa`r=Ï@'üÆ>@<wà6a¿ë>ñöZ˜[¿ãô‰»fY7¿ééY³$°¿ÈŒÌ¡Ù¯UNASNone@¡sœ¾àPowerLawnone?ïíÌŧ$Ù?há&2³\?b3:•TFó?há&2³\?ïªvÂîÁX?–MÈ5?…bO:Ö	?–MÈ5?î·ÞÊasÊ?šÑ|'€S?¤'[ 'e?šÑ|'€S?ïñ:6æ$?H¿@7_^?]ы÷è'ö?H¿@7_^?îcJ¾²i?¯•ûtð?©Ë_Ö¨Žl?¯•ûtð?íÚßñ±wv?ºTq"Ÿ7?±)râ7Ó?ºTq"Ÿ7?éÅs6ÙZû?·[…IÆì?Èê3$š"?·[…IÆì?ïcëfj?‹r×aF)?"'Ÿ–®Ž»?‹r×aF)AGN3FGL J0527.3+6647@b2(õ\@1Ä&5ïÀ:¼ÆŒ@ëƒÀ<Ü<¬X¹?Õð%cß@àà+yU?ý T "žX¿ïy<G׎?è«ûújr¿Ç4A¢D…¿×СõØ<UNASNone@¶téûçl‹PowerLawnone?ïþªMà¢?"·KÈÀh?#ÕX¼nÐÏ?"·KÈÀh?ïÉúÒfD?"7ýÔHðs?{–«N2?"7ýÔHðs?ïß?à¸'?k4šoº†?p`ž|W?k4šoº†?ïÑx`;?^ªy)|?wÄRG?^ªy)|?ïúµý
Ãs?D}¦pþA?E(k|Óv?D}¦pþA?¾hþ>?³.ùÄ?¦&Ñ"?³.ùÄ?ïÄê
X
â? VIé#?}Šù@¼¿T? VIé#?ïëUÎéˆ?F¢€çÔ¸?ž'•M?F¢€çÔ¸AGN3FGL J0529.2+3822@eFÕ䣃'@v @hÀ8éæè¹À;+%Â1?ï&gâ.@aÔ=ÚV"@D¡àe¿àH0…PXտ馃('ÄÛ¿êâ3ß´
¿âxC*¥UNASNone@òSeâXPowerLawnone?ïçޘýŽ?lj²G…»™?h!gîqã?lj²G…»™?î¥,ö¿J¿?°×ö­Ž¡?¥­0—zð?°×ö­Ž¡?ï
ÓØZ?'õøÞ¤°?žPíîÓ?'õøÞ¤°?í»‹¶¤cÄ?H­ÃÈZ?²#¢I%ß?H­ÃÈZ?ï'÷+Θ‡?š'D4Ú ?‹B5‡ê	?š'D4Ú ?âíØçs}a?Ï76&qr£?Ú$N1=?Ï76&qr£?ëÂ`''èu?¬)ÀyÊtÂ?Àö}µ¸^+?¬)ÀyÊtÂ?á¸Áκ?½::A"Ö?܎|c‹ð?½::A"ÖAGN3FGL J0533.2+5944@cõÐúY@,8ðAFmÀ9·´Ï€tÀ;"A® 9?ôw¬NÒöÝ@´¨€èß@¾?–Bø¿Ô:"´`"¿è
‡"¹ ¿ïÿ"[}em¿äüèjÚaUNASNone@}>MÓØPowerLawnone?ï«Ó$ª¯?•¾µá7Ž?…8‹D"Ä?•¾µá7Ž?çS'×¼?ʈd}ò¹?ÑùßXÚPˆ?ʈd}ò¹?í"í>v!3?¡ý*ÏñÌ?³X–¼éå?¡ý*ÏñÌ?絛'Òت?¬ñ·dqî?ДÈúZN«?¬ñ·dqî?îsÒu¶Ãÿ?±o¹.1?¨ÂØ¡$$
?±o¹.1?Ì]"Yt?ÉÊvrðYç?èèº^é¢ú?ÉÊvrðYç?ê€)­ÅÂå?®ø}p?a?ÅÿYHèôm?®ø}p?a?ȳYËų?ºX—†CüY?éÓ)"8?ºX—†CüYMIXED3FGL J0533.8-3754@nYcˆe"¯À>âôðØDÐÀ9ñjÉ¢uáÀ;ÇB??°ð¿ø«md¼@4¤m23@¾÷€—:¿Û·çÉ¿é$ {ÿ¿çô•qIw¿Ão¨{×\UNASNone@þë6z'PowerLawnone?ïÿL`ù? ÒèáFÌÑ?v{­•–? ÒèáFÌÑ?ïӣ椏A?Œ<XÖê¦?v.¨8ÿŠ?Œ<XÖê¦?ï¶sÜ#`?~"].ø¬?'`#ª$?~"].ø¬?ïÿù[1e9>Ä{ږ¹=y>ʔ"œþÉj>Ä{ږ¹=y?ïýÐUB|§?6	'öJª?1}Wlï¾?6	'öJª?ïI";¨ïð?®ì¬Á2‰?–͘…º˜?®ì¬Á2‰?îýv‹«"?—§ú Bx? (—Bº*W?—§ú Bx?ïÿ_Â;?!3Gsˆæ?´MŠ?!3GsˆæAGN3FGL J0535.3-6559@q=Øâe,À@("_õIÀ9ÖÇÉWÍFÀ; dË[³…?¿ti"Ä@Œ!Ûé@˜¾_쥿åèå}C£¿âíɽJÏ¿é¯DI8¶³¿×?°=†/UNASNone@
üÚQPowerLawnone?ïûwVg"?Dhǒ«n`?B"¦3¿×š?Dhǒ«n`?ï̊°Þ?¿«ÄAøn?yº±ï?¿«ÄAøn?ï¹ÚÔø?l?tÄ2îbF?‰J²!ñ?tÄ2îbF?ïåÊö›Œ?TÐÞücŒ?j5	Æ)#ù?TÐÞücŒ?ïݜÆIÐÙ?uüžZ?q1œÔèGM?uüžZ?îïõY¸"?±'+‰ˆ¹Ô?¡¨ÐÁ¿?±'+‰ˆ¹Ô?îñøgI)?—Í"£'¤? ïðzgTl?—Í"£'¤?î@•Ä¢Ü¹? 3.îq?«ö£¶®j? 3.îqAGN3FGL J0535.7-0617c@j=pdìé£À3¯—Ý÷wÀ9Kd'`˜À:ég¬·ƒ?¯+«ãõ½š@
¾‹Õ‹¸0@+Þßsîd¿ãb¡Õt³~¿çi¨$*¿ëE|Ђ¿ÓÕ¾î'Å?UNASNone@Œºw€4mÆPowerLawnone1?ïÍÀ©Â h?"°»â(Z?y«4­Kõ?"°»â(Z?ïÅY{$?.¢û ?}rÓ`ª"·?.¢û ?î†>ØzLo?šiž$#èì?§œ|¦¼?šiž$#èì?ïåm(]¨c?Vì1°Àì^?j'ת–­?Vì1°Àì^?êþ­^aN?Ãng¢âª?ÄJ†zǶ?Ãng¢âª?î©
Ekw¦?°ýéڌ™z?¥o+¤ý¨?°ýéڌ™z?éC½'é4?·¼å#/Úä?Êñ	ô[Ã0?·¼å#/Úä?î!;1%ß?£(rQ5Ÿ?­æ,L»?£(rQ5ŸAGN3FGL J0536.4-3347@mÉ{Ç÷zöÀ=o¼¡ŸÀ8¥»^æ?eÀ;‰al+¢E?ïÔ$
6°|@5"×ëŽÚ@WQ­Dq¿åøó	*(Ñ¿åù?®/—Œ¿âîü"þ"Þ¿Ò¦°UëUNASNone@‡ãy=ÙcPowerLawnone@?ïÿ©FÆõ?]@ÊVXÁ?®F"ðãB?]@ÊVXÁ?ï˙N£¯¦?'Ò¸2?z3XÊTù?'Ò¸2?ïáÁH't?l>Éjrߣ?n>ü™0ü—?l>Éjrߣ?ïö?"FÀ?7Ð_ÏL¿Ô?S€÷"@?7Ð_ÏL¿Ô?ïÿ´|Z)Ó?"L…à?àëãmlÜ?"L…à?ï­Ïå0?±'í
ºÓ?œŠFŒT?±'í
ºÓ?ïÁJ!%-{?€Î²þÊ=?ZïMîÄ?€Î²þÊ=?ï߮݉?ba­Ô?p(ûÿ™Ã€?ba­ÔAGN3FGL J0537.0-7113@qŸIšé$òÀ?ŠµÃ›Ë£À:'q^-À;'lSq?ׄð4m@/ÒxÞ8@Ü )€­¿×
ú7œ¬ý¿ë³»õÔ¿êΚr1 ·?¶:,µÎU#UNASNone@'TIQƒPowerLawnone?ïü½æÞy{?E,왲h?:Ç6¶Vc?E,왲h?ïÌUo^æ?Ù`ŽHI?yÕ?<¡á?Ù`ŽHI?ïH%ÔA?Êëç"N[?–î[L]Ïà?Êëç"N[?ïóMeA*ö?Kt·Òà?Ye4öùdd?Kt·Òà?ïéPúL‰?qy‰—
£"?f¯…0Ç?qy‰—
£"?îàE?²qûlˆÄ~?¡'.ŒD?²qûlˆÄ~?íµEéæ…?«Éet"ÿ\?·ÚU΋
W?«Éet"ÿ\?ï,Áç7ÿm?˜Éè33?šgÃo®V?˜Éè33AGN3FGL J0537.4+3604c@e ¼¾aÏÿ@h›_lw"À9ƒÓQKL/À:à«ÁºJ?à ¹ü*@
ÈQÉ÷/w@+ œ'­¿å ¹8ùÏB¿ã³Ó'7X¿êŽJÂ,¿Ý—…Ó>+	UNASNone@£x}¿HPowerLawnone ?íNҁӻe?ÆÖҒ½?µ‰kï<c^?ÆÖҒ½?ï.›5h(?¥cßüë?š,™S23?¥cßüë?íJeç?§®²©Œ¶?µ¬ÐÉɅ?§®²©Œ¶?î¦f1Éaï?‹Æ)©ùav?¥™œå!¯?‹Æ)©ùav?è¾
_ö?Ê6rfFR?Íʀ'"Ô?Ê6rfFR?ãú*Åó·?Ñ€ìFA?تt'Ø?Ñ€ìFA?æřqN2?Àé-€–¾?Ófçcœ?Àé-€–¾?â$°á+Jÿ?ÂNúd	¿Ç?Û¶ž=©j?ÂNúd	¿ÇAGN3FGL J0538.8-0341@iû}¿H€À1Ò=p£×
À9™AÞËÓÀ;2qúï?ò2JˆÎ@ž'‰±Å
@ƒßà›¿Ùb\ik<¿ìWG†ôž¿çq6Аj‹¿ïÿp'|¾UNASNone@"?,"h	ÕPowerLawnone?æ=8¹É©œ?Ñüþߪ±*?ӅŽŒl¬É?Ñüþߪ±*?É´fL º?ÈååY'õ‹?é'æ{ì×Ò?ÈååY'õ‹?èñ`¼¨:?¯'=†ž?F?Ì:}±_?¯'=†ž?F?×ÜóÖ¦ë<?©Ò±	Å"?䆬Šb?©Ò±	Å"?á0e¾JÓä?Ðs܂ï«k?ݟ4ƒjX8?Ðs܂ï«k?¨G•Šò?¹ôjºLÜ@?î{†®°W ?¹ôjºLÜ@?áá§
¬'?¸—êæo™?Ü<±ê¦Úþ?¸—êæo™?¥äÿì'÷?™ ?€´°?™ MIXED3FGL J0538.9+1646@g³&¿‡iìÀ£¾"åÞÀ:ütðmÀ;t!퐑³?è«ñàØrr@ƒU@m-?þ@^_0çÿ?—µo	¹lg?Ü'§ÂYßοØeo™H™¿âÄz\¬B-UNASNone@±i/Ÿ¾PowerLawnone?ïýÛ¹Šá×?._
€*W?1"1¶Ý´?._
€*W?ï?W'üjÂ?¡ª°ÝÌÝ?˜þºÙÑ?¡ª°ÝÌÝ?ïÔDÌsò§?uí¢	F§?uݙ±i?uí¢	F§?î×¹iºü?|¶´
ß?¢"ie,&:?|¶´
ß?ïõˍvdz?R/Á†l?Thå`.Kg?R/Á†l?êó*‡Æü?Ä<OÍ®Û0?Ä3Uàå¼?Ä<OÍ®Û0?ï«È°³fŸ?ƒðdò=¿?…
Ó϶¼3?ƒðdò=¿?ëh쥪R?¤Z"Eþ¯ ?Â\OõiV¹?¤Z"Eþ¯ AGN3FGL J0539.9-7553@qô¢}ŠÀ>–~
ÇÚÀ9ÐľáQ¿À;Â6âëC?²J…^t
±@SIÑ«@š'@‹¶W¿ç¼ŠM²v›¿àÕ6Ó@O¿êÉâ?Xc¿Þ~ØdÒßÙUNASNone@'¯FÜ]dPowerLawnone?ï÷ÑS«^ú?W!ÚÑ0+?P]Xµç?W!ÚÑ0+?ïÉ 1…«s?È"Z>?{/çWGN›?È"Z>?ï›(]þI-?|ŸQÙ?‰5è|þÏ?|ŸQÙ?ïӥܝû(?_㹕à?v-ɯÊ?_㹕à?ï}wå??˜,ÇBÑ	=?_\-"¼)?˜,ÇBÑ	=?î¨ÁHùÝÁ?³.fŸæ?¥sërõØï?³.fŸæ?îК?£{uo­\Ñ?¯ÓφÂ?£{uo­\Ñ?ìÞsœô†¿?©Žtp–ö9?¹c7±?©Žtp–ö9AGN3FGL J0540.0+1208@h7‡?úÁÓÀ#¬U!š"{À:
ï°ýcnÀ;iþûôÅ¿÷÷äXÍ@œQþ'@ÛQŸÚÑG¿µf#@9¿ì{
jð—¿ÕF"¶U'¿Ó 'ü¨mÙUNASNone@©¾ïhیPowerLawnone?ïÿ)Oüäå?%l¨jZõ?Õÿ줺?%l¨jZõ?ïÃ^ý*/?ŽžutÁàð?~Pöeî–?ŽžutÁàð?ïä¹Any?h°ËÑ°z?kF¾{‰aá?h°ËÑ°z?ïÿøÀ	‰°>ÄBnÅk>ÌÿºwòÓ>ÄBnÅk?ïÿOoÿÂ? ]!ø±L?vèõI? ]!ø±L?_q?²TæD拓?¤×N£)¤å?²TæD拓?ïâQ­¶uâ?t‡Ü3ÆKÁ?m®R\ÇíÇ?t‡Ü3ÆKÁ?ïÿ®–«Óƒ?RQ¢ñ‹‡?ZQî22¾?RQ¢ñ‹‡AGN3FGL J0540.8+3503c@eÈ}¿H€@Þì9yžRÀ9QؗÜ*8À:Ց¡}"ª?×týý`,T@
ßÈß'·@* À){N¿¨Q¾N.â¿ë‹Sß¹¿èҘ–dZó¿á+k4›,UNASNone@
Q¢£YPowerLawnone0?ïãHº·?uÙæD#ç­?l·E#e'Õ?uÙæD#ç­?ï"Pˆiכ?œ€Ü
¦j?‹+ÝÛ;E>?œ€Ü
¦j?îsW³?¡b‡Ë8?¯ŸO: Í?¡b‡Ë8?ïž^
³sq?lbûHq3?ˆh}S##Ø?lbûHq3?îL_,hò:?²n¤«?«:
7¹[?²n¤«?ì`–Ïÿv?À€š¼{¾?¼ûI€OÎ?À€š¼{¾?è´²U
Š?¾gã"•?Í/©6«ÉÙ?¾gã"•?ëçöŠû
?¬8éᝣÆ?À`%Ô×½?¬8éᝣÆAGN3FGL J0544.7+2239@g(-¡"ú×À"ôß:›À9m"š\7À:Ȫ-e"Ù?Ë%Ì~"{‹@ûäêû¶ð@ýÖàL'¿ëd¯N"¿ìiPjjq¿ÐŒ÷£ÿ½Õ¿æÝÎzªsºUNASNone@"¿µÂ\)PowerLawnone?ïùí‰Û¶u?R¼ù˜¤P~?HIÙ%•LÃ?R¼ù˜¤P~?–Æß?š4ß,‰D?‹ßÚQ·Ü?š4ß,‰D?îö~Ëb?– àóÔü? ž'É?– àóÔü?ïÄ/øɳp?dÏéRº›?}茷ëã?dÏéRº›?ïÕçÙv1?|DFa?‹?ue㶫?|DFa?‹?ìR6Öx??Áô'™ˆÛ?½ovIL>?Áô'™ˆÛ?í_¯÷î¨Y?§3:¨¾Ø?µ€>Òï>?§3:¨¾Ø?îxsÝÙu¹?šuy9w§?¨xÂ"h¤s?šuy9w§AGN3FGL J0546.4+0031c@iœuy(àÊÀ,Q3ß*À9g<kÁ:À;!1ZL?ëj¾ÿs'@Îìt‡ç@@ŒTçÑá¿ÞxoÖ:ñ¿ç–¢ˆƒ¿ìxªô_ãÀ¿Ý)1þûLUNASNone@~¶âëCPowerLawnone ?ïìB¹ÁŠØ?l×k'"‡O?c½FIsè?l×k'"‡O?ïz$Ö	²?˜óãvod?»e<ûÏ?˜óãvod?ïT'7}ù3?Š(›m½ú?•mÙø§¦?Š(›m½ú?ïíÇ)…ò?'VnÈê¤?Ÿ¢G#fGÄ?'VnÈê¤?ïJÑüGÊÖ?žCÉï¨?–¥ÀzvA:?žCÉï¨?èùA§a¥¯?È@­³ç×?ÌùbyiE?È@­³ç×?ì;Á"U)?«%c©Ó?¾'ùóeV¶?«%c©Ó?ç^Ù¿Eó?¼¨¯TI‹î?ÑBäLt?¼¨¯TI‹îAGN3FGL J0550.3-4521@o}n—OßÀ=H¤TÞÀ:´ƒ)ìÀ;¤B"ÏÞÀd&Æs@üЉż@C )"¿çbò†ßû¿æÆ'Ûjþ¿ê¸NÉøÃ1¿à"}ÊþcUNASNone@"¦òGE8ïPowerLawnone?ïþädC '?&¨
ˆUÚä?!¹º^d?&¨
ˆUÚä?ï×ñW›?ˆ=ijX?tqL£
`?ˆ=ijX?ïÃåsÈá?v[ÊéŒ7ê?~~[i#'?v[ÊéŒ7ê?ïÿÿþc®â>AIÛXKâé>+r™ÿ@M>AIÛXKâé?ïüx¥Çéþ?@oâÙ$Q?<:ѯx?@oâÙ$Q?ïPx¥‡?¬ñØz?•ðëc[‡?¬ñØz?ïz¹€P³?Š›6[§?¨Ïíh£­?Š›6[§?ïÿÿ2`á}>­Æ€G Ç>™µi¨¥Ï>­Æ€G ÇAGN3FGL J0556.2+3933@e~P]¥@7.jwÀ9-—ïunAÀ;_	ðCÊZ?Hږ!\¡@¶†ü#»@¾| aõ>¿æè'Wގ@¿íbääúƿꄉðŒÎ
¿è=¡íêÃrUNASNone@kœðEwÙUPowerLawnone?ïú'*Å?D¹yÌGl?E»çA®#Q?D¹yÌGl?ï³:á8¥Ê?wGn°`%?ƒ1G­ƒ?wGn°`%?ïhꖦ?(Ό\Ș?'â­&Ô©?(Ό\Ș?ïºcçc¯…?f!\àÅkô?gà¹?f!\àÅkô?ïáP½æ2­?s""úÒë?n¯BOg:²?s""úÒë?íºëU4?¸FԈítÄ?²(§™o^?¸FԈítÄ?î)7h:ë¨?¢$v/pÖ¹?­l‰Àáy?¢$v/pÖ¹?ëÞª'÷O?ªjG\Ð?À‡±U´"Ã?ªjG\ÐAGN3FGL J0557.7-0720@j®›¥ãSøÀ.}Ñ¢£YÀ:->9 ²þÀ;oX)ŒÁD¿ðä/,=u¬@ü‡ÝÚf=@/;ßÕA¿éâ¼"ä;¿Ó õjÈS¿çà´¡ÃðÁ¿ÆçãUNASNone@¨N%`A‰7PowerLawnone?ïúÀa?Ç'?WI8id.?Dþz›.öŠ?WI8id.?ïÈLÐ=D¯?Ž	Ùú[?{ٗÐ߈"?Ž	Ùú[?ïöÁN$·?'ý,;`´?‹ÂO¥—š4?'ý,;`´?ïÿ‡Ì&?õR‰¶?<Ù7×Æÿ?õR‰¶?ïèÝi}5?j%4~ȗ?g"–¬\?j%4~ȗ?îÑác"Â?±µu¿H—?¢áéÅzß?±µu¿H—?îϪÄî?˜¯õÄï?£~'¿ü(?˜¯õÄï?ïò…C f'?[E"'«î?ZõzH¤J?[E"'«îAGN3FGL J0559.8+3042@f!ê5"`@~½à ¿(À:+0/r´À;pê‹út¦?æjÞu–°@
N½u@ô½?û`zßDH¯¿ïÿö(výÊ?ïþ`  =Ú?cÝåÉQÿ¿Þù…ét´nUNASNone@ÀU¤¼j~úPowerLawnone?ïþ¦MÃ>?3¼ú|?/…˜(¼"‹?3¼ú|?ï^Hüëp?¦"•0ÁMo?"?¶ÙƒZ?¦"•0ÁMo?ïÒÔÇÂF?qQþ i~?v•œk0ô?qQþ i~?ïJ+Ì{]?}Å×qⷘ?–º†nܑ?}Å×qⷘ?ïølés?O¦á|a£?NL\:E«?O¦á|a£?ëÜIy'F?Äñg>†+0?ÀŽÛ®¶é?Äñg>†+0?ïœr|ýµ+?†â~Ù²Šî?ˆã`½#\?†â~Ù²Šî?íÝì<SÃL?£P]Юf?±ž%?£P]ЮfAGN3FGL J0600.4-1934@l-1;â.^À3¼˜å>³šÀ9âÆo»y¾À;­1"́þ?ãٍ«d@®Ðǃ@r @§ºï¿è~u΅«ó¿é5Íí3J¿è&s†¬ÏN¿ïÿHÔ|¥UNASNone@"âCWPowerLawnone?ïçë"g!ç?vx8lù=œ?hÝ}a92?vx8lù=œ?îeGá@!?©ÚI."Š?©¦ûƒ£Ëè?©ÚI."Š?ï-¶©lAê?†•-ÔBš¬?šI*˘ŠÊ?†•-ÔBš¬?ëÞ-'?—)]‡Ê®?À‡¯I··š?—)]‡Ê®?³Lø?'üÚHÅÈu?‰œDËùù?'üÚHÅÈu?à_lÞ5ç?Ò)N¥?ßáA&C"2?Ò)N¥?íµT–bàþ?¤Ê¯\Á¥f?²U[MÄß?¤Ê¯\Á¥f?Óo³^33?°a•7³k??æH&Pæf@?°a•7³k?MIXED3FGL J0601.5+2309@gYW)²€ñ?ÂÀË6ʗhÀ9N˜0
À:íÒä>š?ÛËÆe!@—ñ5·ÇØ@àšüI½¿å²y3‰æ¿åKt­¸¿éc™Z¸¿ç€ †eéUNASNone@Œ'½¥œàPowerLawnone?ïê$ûS^?pޝmµ?eÛålQÊ?pޝmµ?ïhO˜Æé? y£™i÷?'öfêÝ? y£™i÷?îћY÷¼?™2¡û®ZÉ?¢æJk@è>?™2¡û®ZÉ?ï/úë)jn?wh´ aY?š¢Ÿú@?wh´ aY?íõÌF®ÔÙ?´!m¶ÅW?°QÈы;?´!m¶ÅW?é;w)Ø?ÇS ŽÞÞ%?Ë'#XŸ©?ÇS ŽÞÞ%?é nÞÁ'8?½¹˜ùœÊ¸?Ë~D"ûc?½¹˜ùœÊ¸?ç´h—:'?±°–6<ñÜ?З.ъÝÐ?±°–6<ñÜAGN3FGL J0603.3+2042@g£ùHUÚ'¿æðí=…À:c–j:0}À;.LC¥q?¨âg-¢Ê@	ºRøöKv?÷ÿŠŸUÆ0¿ï|	›ÄC?ïqlÜÍ ¿µ/µz¸½R¿æb"¬
ÔCUNASNone@ݼŸ¾vÉPowerLawnone?ïØ©ì;ì¯?ªG`Jɟ?s«	Ï{Ę?ªG`Jɟ?qvK?—rÊ#¯oŠ?£"®É
?—rÊ#¯oŠ?îû#ÿŒ?˜°¼®™u? NíÑc¼;?˜°¼®™u?ï£c2‡2?u`ü‰›Ò?‡'3J°'{?u`ü‰›Ò?ïê¥!¯tš?o¾ÇüX€ ?eZÞ'æ´?o¾ÇüX€ ?ëóÔòq]L?Åü)ïñÁ?À0¬6:ŠÒ?Åü)ïñÁ?îìŒO{Š²?˜›‰Ò´êÄ?¡7;kmÝ?˜›‰Ò´êÄ?íÝôÁ¢;?§Ì7µ$ÄÃ?±Yó\Â?§Ì7µ$ÄÃAGN3FGL J0605.0-0000@ió(àÉÙÓÀ$š¾'›þÀ9"àê'À;Xƒ°j?Í*™où@—8v,®@'T"¿Ò@C"OÇ¿âR€"ÁÆè¿Þ{>í¼¿ØèÛ8þ׿UNASNone@¨bp:û~'PowerLawnone?ïþø«šE?)‹á'%X	?.0s惹}?)‹á'%X	?ï´Oˆ(ƒ?'«0²ßœ?'ìþÎ;µ?'«0²ßœ?ïÖÍQà{?v _¥Ë?t™VôEœ?v _¥Ë?ïîyž»'?CÖ8G› ?a†:Šþ>?CÖ8G› ?ïöÁ&ó¬,?R"t4â`4?R}²U nj?R"t4â`4?î"ƒ ^ì?·Šˆr&yl?­×Åý]7?·Šˆr&yl?摒¯G??†±x£c?…\@
h?†±x£c?ï¿6ǒ?{4g›±«?Y'
¶?{4g›±«AGN3FGL J0605.9+2039c@g¯Þ¨—c¿Éß8IÈuûÀ8Àº;А§À:¤®á){?ô¶@K)t@cä¼Î@Þþ€N?ÎR	 pV¿äùóK'£×¿ë%Ʀˎè¿è6­Í>sUNASNone@"7"g8~PowerLawnone ?ã_Å:ºÄ•?Ï;ۛ‹{?Ù@uŠŠvÖ?Ï;ۛ‹{?Ý´j—ðÄp?Ë
ŸrC
ä?á%Ê´È?Ë
ŸrC
ä?èS|­‹Ð?²×é¾"¤–?β
Iп²?²×é¾"¤–?äS	Çn?¨*WdÀÊ?×Yíâq#Ú?¨*WdÀÊ?¸Å ñ{—?½Á¼^¦º¦?ìç[ü«Ý?½Á¼^¦º¦?¶M-NO•Ö?¹—Fu]¹¿?í6ZVQŠ%?¹—Fu]¹¿?ÖirŠar?»(2l8ã?äËFºÏtG?»(2l8ã?Å]̙¡&V?¬Å?J#×Ï?ꨌٗ¶k?¬Å?J#×ÏMIXED3FGL J0608.2-2306@l³­À˜$À3hOô4ãÀ:r(œ×;¼À;áàÈðŸ?àùµI^ª@
úp­½@štŒB¿ä´×Qyß¿ä@¦ñ›ä"¿ÌeÔ
È¿ïÿ£©	pŽUNASNone@˜ÎãS÷ÎÙPowerLawnone?ïäO•ï?y4míÌ?k°jÑ8!?y4míÌ?]{[@?'ËûE×ï?Üh¤˜Ëõ?'ËûE×ï?îj†|dD?—Zš¿¤f?©W˜7+ÖÂ?—Zš¿¤f?îҜ"??†0†ä•?¢Ö>ï¼?†0†ä•?ï¸~ˆéjŠ?‹ÛV'~ôþ?à]¼¶a¡?‹ÛV'~ôþ?êäÍbÚüÍ?ð¢z~ï?ÄlÊt"Î?ð¢z~ï?ì4…åv?®áVMç?¾_ÛÐÔKû?®áVMç?é'&äèš?»'€(aü?É÷›dl]™?»'€(aüAGN3FGL J0608.6+5328@d	 {5*"@/›Oe™À:Ʋ˜¬À;œnCªy¼¿ë½ñwÑó¨@áÖÚAÕ@ðºà'$Ö¿µG㈿àŽæ•ÔF¿é¤Î#"¿ã'èd6¿UNASNone@‹/Ùb¶®PowerLawnone?ïø<k"ø?\½´1£?OQÛàn?\½´1£?ïÔ%l?"&\@‹Ëý?uùíWþ?"&\@‹Ëý?‡[æ?˜ŠVÙÌ'?-èÉíU?˜ŠVÙÌ'?ïü@".þñ?-³MÕQ?=þíҝš?-³MÕQ?ïÃÚÁÀ?‡ñ¼ô§,5?~ñ²|$?‡ñ¼ô§,5?ïÐ[Ár?°È²Mÿï?žåüô‡ÑÆ?°È²Mÿï?ìۏ†"÷Ú?ª†[°G3…?¹#ƒÎZ/?ª†[°G3…?ïÔC[ó?ƒrP5ì°Ì?ˆŠï6øóC?ƒrP5ì°ÌAGN3FGL J0609.2+2051c@gµzáG®?âÎìóàÀ9-J´O(À:˜}–-ÔO¿ãoXš9Á@
n¹?!@.'`@3¿Ò1#"Øå_¿äÝ÷½l4¿ë°²@jºo¿Úð¼UNASNone@¥j#9ÀìPowerLawnone0?í«ð֎º?ÄïR»B?·Ú xݖ±?ÄïR»B?ﲁ"Fmš?'oü5qÜ#?ƒ_žã½ÏŽ?'oü5qÜ#?ꪟײj1?¯ŽwYF?ÅU€¡6W;?¯ŽwYF?ïú_k?:VÖz®?Fƒ™X	÷¢?:VÖz®?äa
_2<?Ð'¦b)ì?×=ëA›Åˆ?Ð'¦b)ì?íåÚ']?¼HBµ˜cö?°Ñ/
,åñ?¼HBµ˜cö?æ^[,Böl?¹"!Ö3™?ÓCI§z(?¹"!Ö3™?ïl&t¼s?Žnj§úÁŽ?'{1eE?Žnj§úÁŽAGN3FGL J0609.6-2851@mnµÇ͉‹À5/.ÌțÀ:J¥öŸ..À;æ,_Ú[+À"¦ÃMÈ@	A–xQö@ý`O¿èT-ĉ\`¿æZýñAѿ㜒i=u¿ïꆳ&Í8UNASNone@4ÔɅðoPowerLawnone?ïúc¤°?SÖ´à¥zV?Fs¾.åç,?SÖ´à¥zV?ïÏ*
Ѧb?Œ³Î_Z>Ì?xjúšœk4?Œ³Î_Z>Ì?ï…ý$Oâä?z&Åq¥½÷?Ž€¶ìG?z&Åq¥½÷?ïÿêáµ½>âÂø¦éw>åˆ"¡>âÂø¦éw?ï÷Ü0©&f?VAÎ'"?PGžp ›e?VAÎ'"?ï1¡-ÑÅ?­H´ãl¹v?™ËÚW¦^?­H´ãl¹v?ï[¬5þi¨?Ã î»s¯?"ŠyGú?Ã î»s¯?ïý3‹·rŒ?7ÑOš",?6c£4(æ?7ÑOš",AGN3FGL J0609.7-1841@l.ÄÑ¢À1bÑ9C­À9¢aÅíµ{À;›ÀoÇ88?ç	ů)×@~ÛËÃ7x@cËè ¿Ó;ùæ`q°¿å©O°´¿ç"Ky¯n¿æµêpLšUNASNone@'.ïiDg8PowerLawnone?ïúŽ.+Œv?QÙ9Ux?EÇGsãâX?QÙ9Ux?ï"ä;±ås?'
Ÿ$óÕO?‹ñ	7Ï4?'
Ÿ$óÕO?ï a©/o?'£H^¯?‡ç•Êø@?'£H^¯?îü2ý?uS™ žD? <Ð'
¶?uS™ žD?ïÈ'Ëdܒ?ÊË(|‡Ð?{ìF²~Þ?ÊË(|‡Ð?ë'#Y)²?¿±â³
{P?Á÷r›[™6?¿±â³
{P?íì¹~]ËZ?¦|ë,0?°š4
ëã¶?¦|ë,0?è4zOw?ª¢,:E¡?Ï.âÂ#ô?ª¢,:E¡AGN3FGL J0611.5+1957@g×.œË}A?丝jßrÀ8Þ$ZR[íÀ:¾Dä5Ÿ?ôjÅ(=¶Å@³ÅPÉ@e@v'®¿ÂtÂvÔêö¿èvssârH¿æˆÅ(
,¡¿éœuʐUNASNone@"¿@PowerLawnone?ç‹©…¹­?ÈC¦ÏHcW?Ñòè¬ôŒ§?ÈC¦ÏHcW?Ûó,u²gN?Êú	NåI?âiÅ&ÌY?Êú	NåI?êAçåñ¥¹?®G݊_f?Æø`h9i?®G݊_f?ä†îoŽP?£¯Çb½÷?Öò#!Üã_?£¯Çb½÷?ÄdÞ¸ð?ÂØ¥
¥ÿ?êý&ÈQú?ÂØ¥
¥ÿ?²ÉÅ}C
?¸v<f*?í¦ÇPGQ^?¸v<f*?ß. ‹jÀ?¸Ôz«)Õ`?àh¯ºJò ?¸Ôz«)Õ`?Ưô'{ùS?¥4Ái–l?êTßa«?¥4Ái–lMIXED3FGL J0619.4+2242@g¥Ô¿	•«@l'"øÀ8åtË"¾À:dX R…ß¿´j摏¢@Â]](O@ƒ 0w¿æsñœ÷¿àr¼‡Ò".¿ßNr\q¿äI͖ÑOUNASNone@·È1&éyPowerLawnone?ïác-ˆ	µ?¦Ù³eÁ?nœÒ¢'rS?¦Ù³eÁ?ï¸$.æûÖ?'åOpB¤?öôIº'?'åOpB¤?íœÃò!‰×?¥¸q3ê€K?³àqrÃ?¥¸q3ê€K?ïô²>¬
:?BÈöÄæü?V›'X.&?BÈöÄæü?ïœÆéͨY?†×‹–i?ˆÎE~×yä?†×‹–i?îYCiÐíÞ?¶<øÚ3ø?ªkÉb;)?¶<øÚ3ø?íÀ0n1?¥4k¾%PX?±þ|ŠN©Ú?¥4k¾%PX?樓§})?uȖÁ©×J?†œø£ß%'?uȖÁ©×JAGN3FGL J0623.1-4143@o1"…]¢sÀ6ªk\šÀ:…vWu1ÛÀ;âº5"¿ã¥®éjšÜ@©'#Sl9@R?'Kõ¿í^¤blÔ?Ï(²aøª¿äc•åHÞ¿è˜Ò?05UNASNone@–+IºPowerLawnone?ﯷnt=?¢jšO7zß?"$nÒ?¢jšO7zß?ïÉHí?ð?ŽhIÈÿkc?{[‰hGØ?ŽhIÈÿkc?ïÖäÂ{ª?"FAs`÷q?œe#pG¸?"FAs`÷q?ïë®2òŠe?Riñ¬œR÷?dQÍ:Ðr^?Riñ¬œR÷?ïuV
ùƒ9?™E}7¹)Ø?'U>_üß?™E}7¹)Ø?î܏¯ØAÂ?°.?ºr?¢7ÿGÞ?°.?ºr?îÀNS	?¢'¹7…¦?¯û_ƒx?¢'¹7…¦?în‰z_%?o›Žç?©hZ³?o›ŽçAGN3FGL J0626.8+1743@hLœàuöý@
eä`gIÀ9;\Í`qÀ:~·îï6"?ôKg<O;§@&X¹Õy@˜Ëßçܞ¿ÛWÈ¿în…(jϤ¿çm+?Úò'¿ÄÒ*Þê aUNASNone@ˆb¡µÇÎPowerLawnone?ìâÚ½ü$~?º6Hãþ?¸é*Öª?º6Hãþ?îdÇ2Œ£?½'c/
°?®¹³ˆ‹²Ú?½'c/
°?êÖÃ1Ý6–?¯=µÉú*@?Ĥó8‹%§?¯=µÉú*@?îč"½Å?ãnUÇR}?£·-д5?ãnUÇR}?è¨õ÷µÐÿ?ÆUNÆ·‰ð?Í\(!(¼?ÆUNÆ·‰ð?âa#[yÎ?Òµ3îÄï3?Ûù=¹Ic?Òµ3îÄï3?æ=MéAø?µÅ'Š?Óͅd-|?µÅ'Š?éî%b??ÀšÑ
_u?˔GjwÃ?ÀšÑ
_uAGN3FGL J0628.4+2429@g'^_0çÿ@ÔÃ\á'fÀ:û¥þ+êÀ;\nªƪ¿ÛLçDd@
ç݉Þe¦@¨‡Ÿqü¿Ýp_
ô¦¿Óø¬
ÿI¿æ=î"2	¿å‡†UNASNone@ ëËIºPowerLawnone?ïû&™i??L¨‰‡Ý—?Ce™…'›?L¨‰‡Ý—?ï¾û¤]‹?èß!ð?€A
?"?èß!ð?á9ôÌ?'Ó܊~Ïa?ŒX¸bø?'Ó܊~Ïa?ïö–ÛàLB?=‡¨€2|º?RÒHl|×?=‡¨€2|º?ïÒÛSŜN?{†a˜KR?v'VPà?{†a˜KR?îžGšHk?³ïol§ý?¦‹'ëÝR?³ïol§ý?îJI1C¼:?¢jbQt?«[lï3Ø^?¢jbQt?ïiVDҏQ?†UW''|:?'Õ7nEØ?†UW''|:AGN3FGL J0630.2-0929c@kaЦv ïÀ!öúaZëÀ9¤,ŽÔCºÀ;5,)Bï?ò>»Õ-Ä^@!\q@ñgya¿k²ú•gC¿ìÒ
}¡/T¿âu	u…ÏI¿ïÿ'?¼UNASNone@ƒü‡?úÁÓPowerLawnone ?ì'Þu¨ ?»äõãq~ó?¾ÁWÚ»?»äõãq~ó?܃#´BÅÖ?Ëcgƒqäõ?á¾n%ޝ?Ëcgƒqäõ?èVë-NÜv?±pÞáu›ü?ΤSJĎ)?±pÞáu›ü?䭘¼ÏԔ?©Ú£É"˜?֤Ά`VØ?©Ú£É"˜?ç+`V{?È3Vw8¤??Ñ©?SýÙ	?È3Vw8¤??·ØXãRÍ?¿¥Œõyò¾?íôã[w?¿¥Œõyò¾?ášC†£®×?¸×8±ÆbÛ?ÜËxò¸¢Q?¸×8±ÆbÛ?ÉVÔ|]bv?®qØÁiðž?éªJàè§c?®qØÁiðžMIXED3FGL J0636.7+7115@añ~|áœ@8mDþ6Ò$À:
{À;ÑïSàQå¿øwƒ…*L@Ùº÷7Y‰@ڊ ,…Å¿êûRAsñG¿äNnU>¿ãš'"¼²p¿èèÎ̶IUNASNone@"ýŠüPowerLawnone?ïÿ&ÑŠ?ðfà E?%ÕlU]ó?ðfà E?ïÝ KÇK%?æ¨¾—)?qoÚu?æ¨¾—)?ï驟K4\?jÌó5Þ³{?fV`•/<Z?jÌó5Þ³{?ïÿà$îKø>äà¦ë¼Ö>ïÛ7úà'>äà¦ë¼Ö?ïÿ]$À¡?m'b'Ž\?[i陑ì?m'b'Ž\?ï:OXqŸï?­$ꖜ?˜¶줘 ?­$ꖜ?ïÆä3¬æå?'Ñš&³N?|æ5ë%©?'Ñš&³N?ïýn˜íÓ?2ê2cw½U?4‹6wµ(?2ê2cw½UAGN3FGL J0638.4+5704@cÍ|ßýa@4ϋ&9O­À:Á=L'©À;íó?']<?Ö䟫›=¢@}'ûr|Ÿ@jÎ]=s¿ìN^·'ËA¿éÙQ®¯'¿Ë	àØ·*"¿ëH©2øUNASNone@tÒéDg8PowerLawnone?ïþP²ÀÝ?%]L3;-y?*ÿ3³ß¾e?%]L3;-y?ïÊymKªE?ƒ¼r£ºõ?zÃIlÕz?ƒ¼r£ºõ?ï¹°#ãxÐ?€ôfžŒsô?"÷˜
?€ôfžŒsô?ï¿V™·'?d}·4ë?€*YˆóJ?d}·4ë?ïþa.ïÔ?,8®æÉ?)ívc"ó?,8®æÉ?î'1Ú(ç?²yͨÈÔ?¦Üâ`á*ù?²yͨÈÔ?Î	Ó?‰ÁÀ،n?ˆ~Â.·n?‰ÁÀ،n?î¨zKåJŒ?›çŠà›?¥x[=_ÔH?›çŠà›AGN3FGL J0639.9+3250@fÁª:э&@(9äSÒÀ:
¬í#À;ˆðÔéÒÀw4x­Ç@6 \@ó@*·àŠ"¿ãÊ´p×ÐÙ¿æÍó3F‡¿é‡¤t>d¿ãžnÖRªUNASNone@€¶E¡ÊÁPowerLawnone?ïÿE@ÏB?!»/ésö ?^34‹é ?!»/ésö ?ïÓ2»zP9?…ÊŒõ(?vf¢Vş2?…ÊŒõ(?ïζMs?,?oßÅêYÌa?x¤Ù'sîW?oßÅêYÌa?ïÿþ+Ù;Š>¯_d˜Ç>­CÒÇ!Ž>¯_d˜Ç?ïþ0l¯UÄ?/Ê£LTÓ%?,ù4È«HL?/Ê£LTÓ%?ï膴$?°§¢9v?"ï);†?°§¢9v?"­
T?ˆbÅlè(?‹—[_7?ˆbÅlè(?ïÿ A("I?  ¯0=<?ï»êI?  ¯0=<AGN3FGL J0644.6+6035@ca…H©¼ý@6˜)à¤&À9¬Â7G"êÀ;߁SQ¶¬?­e±p›@eyþ§@63Ÿi½3¿ê…wßƶ¿à­¦t|¿àƒ¥p´À¿ÝŸôôÖx•UNASNone@'2ÿ˒:*PowerLawnone?ïþ¹•Å?%9 !X–?$f²oL"?%9 !X–?ïÖË¡(¯!?'æXr0–Å?tš/VZÛ¾?'æXr0–Å?ïØݤ‹e#?woCó]yë?s'-Ÿ€zm?woCó]yë?ïñ1€«Œ
?BcQ'?]œþÄdË?BcQ'?ïø'ê9*?T7‹†€=?M´Våu¼á?T7‹†€=?ï­éÝ©¿?¯0§•?H¿?ŸJBÉr2?¯0§•?H¿?ï^'LÂrÎ?'×'—ê/?";k!B7?'×'—ê/?ïk"¥R¤?'•>)Û@?'íŽÅGv?'•>)Û@AGN3FGL J0647.6+0032@j€Îš,f¿ã"‰ÝŽæãÀ8›èPðÀ:ñ#±µð?ì­½Dõþ@.{ÏÚm@¨Ã ©-`¿ÚPâǜ'¿ê½"6± ¿çߕÒ9É¿âVxÄPÁ'UNASNone@…)*0U2PowerLawnone?ïâ…fîW?n½¦çOwê?mz™ïé…?n½¦çOwê?íËIí	?º}Øó̕ð?³¥·è—·?º}Øó̕ð?î¢NôÚ²é?˜¿²¦éŠß?¥Û´è†e?˜¿²¦éŠß?ììö;Â4)?'¤|
Ò"?¸˜N!î^º?'¤|
Ò"?îèRÅ}UÊ?£Å>ÚxŠj?¡zÓ©âqb?£Å>ÚxŠj?Ú2m1þø?υîtߝ?âæÉgƒø?υîtߝ?é‹ð'Î?Ø?³"ø4£ƒz?ÉÐ=ôÇŸ?³"ø4£ƒz?ÞSm ¥ù?¸ƒïó1TP?àýÖIo­?¸ƒïó1TPMIXED3FGL J0647.8+1751@h'çÀn¹@˜Ôw¼À9Ži°ÂÀ;3è?ïÚ?óàÆ>hE@
»þ5¥~T@Ÿ\"¿ã†3é!ӿ죃äY9¿Ý<è7'¿äà劫6œUNASNone@"'5 ÝDPowerLawnone?ï_L;Ýb?ž«q‰T?"}{óï»?ž«q‰T?ãø…5Śæ?ÏÇ>Kçu?Øõ"tÊ5?ÏÇ>Kçu?í¹;øvR?¡TCŒa?²6 =+<k?¡TCŒa?éOYv‹D?§Røh"?Êš%ÒïÉ?§Røh"?î±0ÿ?²Sÿ"!?®Ÿ£5"?²Sÿ"!?Æßìqö?Ê71ÃO(:?êH;㿃?Ê71ÃO(:?êôo¸—2?­ÒJ0"Œ?Ä.A£÷8?­ÒJ0"Œ?ØëC-YÝõ?¼€"‹£óÌ?ãŠ^iS?¼€"‹£óÌMIXED3FGL J0650.9+6524@bĆnCª@8s¸<òϖÀ:+gÔûoxÀ<µ¬õ–ðÀÛ²t†å@Ó,8Ã@R`E:¿ê£É²ªÑi¿ãd1_ô\^¿ãƒš"ÉÙ±¿ìH¹IY²›UNASNone@ƒìÕßeUÅPowerLawnone?ïîÌãí?a ð?9ì?a~2û÷Òö?a ð?9ì?ïÝß'Ý"?‹Ýç¤Ûì?qlOj%?‹Ýç¤Ûì?ïC«®çV?ˆ>æ‡Ã_9?—œJ'±:?ˆ>æ‡Ã_9?ïÿúñš®å>Å®=ÿ»'Ÿ>Ä9J@Ë^p>Å®=ÿ»'Ÿ?ïà8½
âÝ?rœÕí¥Â?oÇBõ"ü?rœÕí¥Â?ï=7b0»y?­$Ö6ù~k?˜Y¹èð?­$Ö6ù~k?î"^¬\?œÈ|Ş;\?¦Ê£'qL?œÈ|Ş;\?ïþõôìp?&–[Õ¨@>?  ½RJË>?&–[Õ¨@>AGN3FGL J0657.6-4701@p
:æ…ÛÀ2|?>pÎÀ:`%wˆÍ™À;µ£@âH_?äɝ¶gcD@
!¨[Ô<-@ÄÌ>?î3¦p¿áù¬_ç>¿Æxä ªV¿ê
%Á8L«UNASNone@ª?b¶®}PowerLawnone?ï¹Â,úxÆ?™‡ZP#F?tÁ¹Äj?™‡ZP#F?ïFœ¸n,??ŸQ½=Ž½?—,hð'ª,?ŸQ½=Ž½?îXÍàâÈ&? c6-3v?ªs!ð¯ª? c6-3v?yMÒN?‰'ÂöåC?¦%8jFô?‰'ÂöåC?î³ >'?¦Å&© Åÿ?¤ÅþìŽË?¦Å&© Åÿ?êÀvÔ·k«?Å#'Òç)V?Äþ$­"QR?Å#'Òç)V?íg|3ŠÏ…?¥gßܼŸ?´ÄdwX?¥gßܼŸ?êþˆGÑi®?°ûGéCh?ÄÞàºYG?°ûGéChAGN3FGL J0658.8+2318@hÈÞ*Ã"@'äË:%•¼À:`e)O…À;¾eÌ³mÀtóL¾J@lõvº@ZË`6¿è‹á··ß!¿çOY ˜&¿å©MIg…©¿°ã€("lUNASNone@˜ÏÖ8†YKPowerLawnone?ïþÍ·¹,?'ƒ5Ò6ý?#$áín:?'ƒ5Ò6ý?ïÑ.:zû?‡[‹:2
Q?wuhúÏÆP?‡[‹:2
Q?ï͛	Â\Ã?o´§Y¦/™?y2{ÃÍ?o´§Y¦/™?ïÿþ"vóZ>¥»Ü¸;ñ>¦ÄmnL¯ò>¥»Ü¸;ñ?ïûxîö¶?E"Tä"N?BD0¿ç?E"Tä"N?ï
Z‡œ'O?±Zü Eœw?žT¯ZN ?±Zü Eœw?ï:ÈBÏ]v?"åæ.\Z?˜¦÷«;»??"åæ.\Z?ïÿÉI"$"?nâÞð[=>û[:A˜÷Ö?nâÞð[=AGN3FGL J0659.2-0439c@k>§æšÔ¿ÙWŒc¦¬À9-QîÊNÀ:ÙàU?Íu?ÖZãü>Ty@
Ïd9:‰>@3ÛËÍH¿å¯ÀCkSz¿åЬçef¿ägX6Lî¿çf.:ÙxUNASNone@'þÓ&Á¾PowerLawnone!?ï(-—N!?Àk.ßC6?šúM;ß2?Àk.ßC6?ïSƒt¶'«?©{ûyãÀ?•'bPr­?©{ûyãÀ?î€â‡/oë?œ'ù^Ê<"?§ñאxF?œ'ù^Ê<"?ïQ&Í'E?sz}®YT½?•Û&[þ;V?sz}®YT½?ì¦ìˆ lÔ?À€õ2òq?ºÈ›¾ü™]?À€õ2òq?èە7½º?ÈbZL@+?̑«!	´?ÈbZL@+?é5´'÷ǀ?¸Ô'®Þ‰À?Ë)-´ â?¸Ô'®Þ‰À?é"u>µ6G?ª^×=³?Éî++&ä?ª^×=³AGN3FGL J0700.6+3557@f™³=¯ø@1C'·þ	À:NGKîëÜÀ;Úa¶Ô=?åß*¯ø>@ÖшsW@9¾ Œ'u¿åˆ=^¸ÐŸ¿Ý°… à­!¿êð
-ð¿ïÿOÇF.UNASNone@ŒêM:'£PowerLawnone?íòtëJ¢w?±7óèÐë?°lX¦ßÉ?±7óèÐë?êÛΓ²‹?Àua~Ó£3?Đű5Ó³?Àua~Ó£3?ì³]©Ã!?¨7ø¢[?¿e±æö?¨7ø¢[?è"K€M¶?£?MtÁ¸?ÏvÑÿ¢É)?£?MtÁ¸?èêœ[ôP'?ǂҢú–_?ÌUŽ.¿d?ǂҢú–_?ÔV˜ÍÄÐ?И8ùú5?åÔ³™}˜?И8ùú5?æÌ*rfÇ,?¼5ñ'ÓsI?Òg«2q¨?¼5ñ'ÓsI?Á¾pFN2?¢&Àç™àD?ëcüîlt?¢&Àç™àDMIXED3FGL J0704.3-4828@p-xÔýó¶À1ô®…¹èÄÀ:áH2ŸÀ;Á™úèi¿ÐàF9Ó5@
¸ƒ«R?ÿ–Ÿ‹Á?äß5eù•>?Š9¼Ç?ÐƖ4èȉ¿éåH3ûUNASNone@±!˜FÜ]PowerLawnone?ïÝ¿Q Aæ?qÈ}Úê?q W1îÑ6?qÈ}Úê?/
}(?†­Š‡å?€Ü=f;•ý?†­Š‡å?2¨ô?šMX^¢?¤FŒãE¹?šMX^¢?ïãMŒû¦?^ò
–œ?l²rö›?^ò
–œ?ïg++ì†À?—!Nn?"š‡–'ñ?—!Nn?îw÷ÿ;ì?´Ñõxw?¨€€
Äs>?´Ñõxw?í]û&¸?©¼4[ÕJ?µ $ùÀ?©¼4[ÕJ?ï‹)‰Èn?ÕÓMó½w?5¾
ä'?ÕÓMó½wAGN3FGL J0705.7-0006@jÕQ—¢H•@	Â?«ºÀ9ñ½V7D:À;Z³˜H`Â?êN¤d'•ˆ@ÛÛÐö¨@/² %ÏÈ?뗩Ás¿á0DZb–¬¿å·TѤ´¿ïÿ÷ç­£½UNASNone@˜º)Çy§PowerLawnone?íÏóuƒé?À)õ
ÈJ?±€dUŸV¸?À)õ
ÈJ?í«Öªh–9?¸˜$#2І?²¡J­)A¸?¸˜$#2І?éK6(þHg?¯îÈ?k£?ÊÓ'\Þc?¯îÈ?k£?짃P›½¥?•ŠÜÏ×ê?ºÃå{"Ø?•ŠÜÏ×ê?çˆ÷sÍF?Ïê'=Í?ÐîÃet?Ïê'=Í?ä9ùtåI	?ÌÇ
•X±?׌
5mí?ÌÇ
•X±?âV2Þñà?¼ç)ç§f?Û÷SšB@?¼ç)ç§f?á°#fêù;?³"ïëȬ?ܟ¹2*
‰?³"ïëȬAGN3FGL J0707.5-3111@nVúñ€À%V"uÀ9Ïi,êCÖÀ;"ëžI+ÃÀ‡¹-2¾@Z±ƒED@±ù`~šæ¿ækMÿm'¿é|áp®úæ¿ç«Ø)2…¿Ú•2c¡ÝWUNASNone@z§
|ZÄrPowerLawnone	?ïýóØI<?4gɁ–	?0a?½A:?4gɁ–	?ïÉT•·‡?râQ——ú?{Uµ"eøY?râQ——ú?ïê:ëR8?p壟y§?~*âwÉ5?p壟y§?ïÿÿÿv¡>-Ò{fV:>(jl¨§>-Ò{fV:?ïôÜ0 `?\ÔY+'ò?VGžC/Q=?\ÔY+'ò?î±jÚ—Õ?³¢qߊLq?¤éWê7¦?³¢qߊLq?ï4tÉ.?'Ì'ã:~?™q/qBõ?'Ì'ã:~?ïÿÿ©T>›¢eþg¥K>…‹"9öã>›¢eþg¥KAGN3FGL J0707.7-1035c@l|"µÜÆ¿óñ'©"áÀ9/%Ž/LÀ:žYò»?í†ý1é@ÚHtñp@ôCÀI0Ë?èÞKb©î¿çÐgõ¿êû\˜1e¿éª{"œ UNASNone@–»ú¬Ùè>PowerLawnone ?呗•ï|5?ÏÊr'Œ"?ÔÜÐÔ!•?ÏÊr'Œ"?ì‹w&Ÿsp?ÀÑ\ɯ‹ô?»¤FËd'?ÀÑ\ɯ‹ô?çÛ»d³M?´¤-EƒMð?ÐHˆý6™g?´¤-EƒMð?ì¼ìbœá?±êüÁ9Ï?¿rœëù?±êüÁ9Ï?Ú¹~µ×V­?Ò	ýæ†m~?â£@¥T©?Ò	ýæ†m~?ÛøÚfœö?ΦûÞC}ê?â'õ̱…?ΦûÞC}ê?Ú‹ä$WM?½rïÔÂB8?âø:
íÔY?½rïÔÂB8?Ýß«‹"w=?ºñ$"§¨Y?á*:nÄa?ºñ$"§¨YMIXED3FGL J0708.7+1747@hÙm›äÍu@'y»à~íÀ:d«Ï&CaÀ;·'ä™r,Àï a^ë@ÖúM8—÷?ýc8¢gI¿êD0¦2{ ¿è
¾Äî©c¿Èú‰ÏÞ5f¿¯P8ï—ÚUNASNone@µ6_Ø­¬PowerLawnone?ïÿ»‰Ù])>÷øš#ÆïÙ?™qs>÷øš#ÆïÙ?ïп1ûò÷?‡u´õÜ×?w gV˜C?‡u´õÜ×?ïòF~"…‰?Uƒr?V?[sÖôîÕ?Uƒr?V?ïÿÿ¿	âú>7Áú‰X¶>€H-û¢³ú>7Áú‰X¶?ïÿÇïK">÷usâìÙ>üjï	¿>÷usâìÙ?ï:&}©_?±_Ûýâ?žx»)kœ!?±_Ûýâ?ïôPx#¹T?^ovµÍX?W_U˜˜Õ?^ovµÍX?ïÿüLõ¯£>ÄÀµîƒj•>½ša•"ÂC>ÄÀµîƒj•AGN3FGL J0712.2-3806@o0¼¾aÏÿÀ)0HZåÀ9ÚÊ÷àÀ;uÕ`EK?êUVß	æ3@Oþáqõf@5SÀqt·¿äÆ1ò/K·¿äŠ‹ÅN0î¿åƒ¾`£Xà¿ïÿȏGÓvUNASNone@b¨ÁTɆPowerLawnone?ïXx
Âj?œ¡Úlî®?"ðþ§²®`?œ¡Úlî®?îÝ©ÿËÛ>?£¹Fåüû?¢%`®—&?£¹Fåüû?î/Ìd®;£?œ#ô½0ìj?­9µø,É?œ#ô½0ìj?í]([z
?Œ€žtx7?µ.»la¯?Œ€žtx7?ì`'ÿÊ(?Á<"VR?¼ûè)®¿?Á<"VR?㠟†²P?ÎyAŸÝ€y?ؾÀò›_å?ÎyAŸÝ€y?äå^{áLâ?ÀEŒ*Š?Ö5C=f=?ÀEŒ*Š?á›ßX"jL?³¦–OÍå?ÜÈAN÷+h?³¦–OÍåAGN3FGL J0714.7-3924@o^ {5À)dBÇû¬´À9æxT¥sÂÀ;e?åë€@
}ŸVœïº@œÀ? ª¿Ç/I=O…"¿èšÿ'_I¿ì¶yš†åž?Ê•—R+UNASNone@"%Á [ÀPowerLawnone?ïê¢t«ñ?soôÖÀd^?eâ]|5Ç>?soôÖÀd^?廊øz?—r‡#M̌?†ÕÁïÍM"?—r‡#M̌?îò¥Sáÿd?"…òó¨é? ÕªÀ(;Ã?"…òó¨é?ïÜhwä?enSNjsø?qËý,³?enSNjsø?íÚ6vxq?³Ï(M7QŒ?±.LK`3?³Ï(M7QŒ?ì,'¹Aø?ÂK³zÉÓQ?¾žÇZ5ðA?ÂK³zÉÓQ?ëÄbE?²M¬^–"?äîvë™Â?²M¬^–"?í° ©‹Þ?²Bí'û?²Zûý{'?²Bí'ûAGN3FGL J0716.0-4525@p
quŽÀ-âÏ d#–À:G8£µ|À;Á'²D‹JÀòõ¼Û5@
'1µY¾@åÔܑ¿ì;lÁnþ¿â2öà´¿åM‹\¦/e¿Ý"ÙgK#üUNASNone@)Aò×PowerLawnone?ïûÛÒ ?M´-"µ3?C"'$'†s?M´-"µ3?ïÊ­|"??- F1í­?z©A–Dç?- F1í­?ï›X§û å?'M½ÅYL?‰)ÖfšÒ?'M½ÅYL?ïÿÿ<
È0>žŸ¤¹'#U>˜ƒÅ00=>žŸ¤¹'#U?ïØ«¯ÿ?zA"T¥Xž?sÿ*"äC?zA"T¥Xž?îÑ69´ü?±ÙרA(ô?¢ìœcA?±ÙרA(ô?îT'ôÂh?£'âÛ ÝØ?ª¿–Îü†?£'âÛ ÝØ?ïÿÕ²Æޙ?U‡‹ë·>õ&"­uó?U‡‹ë·AGN3FGL J0718.9-5004@pUS÷ÎÙÀ0Vy_goÀ:¦ý/À;¡0-Å5)?ÈN‡Jj:@q¯åC;@"FÀXË¿äbîpFË'¿æeÔñ–¿Ü~;)vÆÜ¿íÊö´Ò°UNASNone@Aà
qvPowerLawnone?ï̓ô`†ö?wiK®&?y¶½.¡5?wiK®&?ï‹v§bk@?'…ŒëbŒ?"V8";Ô?'…ŒëbŒ?î…sf¡l?—@†(D?§¨É—¡y?—@†(D?ï]#‹d<?´A¸¤?Ÿ"[ŒÛª'?´A¸¤?ïGÀ]þŽ?ŸpB@ßr?Ÿwòˆ`F?ŸpB@ßr?éäfûÓ?Ljã¾Ö¿ë?ɼng´¶?Ljã¾Ö¿ë?ìÅ:Ú§?«§Ðåœb³?¹Ö/!*È?«§Ðåœb³?ç5/Û¡;?¸Þ*U²?ѕ H½çŠ?¸Þ*U²AGN3FGL J0721.5-0221@kOuŽ!–S@c)ÞÛhÀ:Pc–¨M'À;YeΑÀ¼Š`Á‹Ñ@
›ÔeÈ[Ï@w í?é¶æà/'N¿Ü.Êz¯k
¿áÜu‡t0²¿Øú•aˆºUNASNone@¬¯+C,¥PowerLawnone?ïþ§Õ
wÂ?"'ʾÝõ"?%'°m—'Ž?"'ʾÝõ"?ï€Ð[3?Ž†ôtˆG?~ñ¿w†¹?Ž†ôtˆG?ïÖLÞßÁ?qøO¾€>?tÙð'ѯt?qøO¾€>?ïÿû¶¢Çs>¼ÌšÃxë>Á%'Æ[±F>¼ÌšÃxë?ïü`šŽOþ?8¬\o?yU?<û,´+Y•?8¬\o?yU?î¢øZš*c?µÍ)–ùÂ~?¥ÐzRí½Ò?µÍ)–ùÂ~?ï¯gb‡+?ƒ~¸4ià?":æ+%Ç2?ƒ~¸4ià?ïÿš:ºwF?¾Xƒ·–?	qFPž%?¾Xƒ·–AGN3FGL J0722.2-2648@n9XbNÀˈ¡ú'+À9œÝÖ³ÖÀ;R¡w´l"¿ðóaHDg@
ˆÝrâJ¸@œÁ¿êPGÕpy)¿àՎL"¿å!ÙJåÀ¿ëÊ}^œåÌUNASNone@Š~{žäPowerLawnone	?îz¡ê©Š0?¯oªz?¨UáVCCý?¯oªz?ﯰ1` )?'ç7;"o'?"ó§×õË?'ç7;"o'?í	N-	£m?£V:­Ò•÷?·µŽ˜ŽË˜?£V:­Ò•÷?ïüD˜¦`?1ÍË@I ?=ÛAHQ{?1ÍË@I ?èñ;äT?ÇL)É8T?π;n¯ƒ?ÇL)É8T?íÖ>˜—'?»]K÷5'?±N;µrD?»]K÷5'?é_ÅÚ·"w?±,C£ëC?ʀè•!²$?±,C£ëC?ï¢ÎR8œ?€·U¥L¢ê?‡LkvB<ì?€·U¥L¢êAGN3FGL J0725.4-5007@p\å@ÌxêÀ.ɶ'!%À:¼šTª|@À;ØúËÙ,?í+žMÒ@x³yi£]?ÿ€@W3¿á,s©£…‰¿ïÿ·¯'C?ïûûU˜°2¿Þ«úõ—UNASNone@µ¢a‰7KÇPowerLawnone?ïôÙp@§1?gtªä}.?VM ¢œK?gtªä}.?ïGqßnÌ?¤±óš¦eÙ?—ߌ©,p?¤±óš¦eÙ?ï‹&nv!½?"ǘçêÙ?6deç,Î?"ǘçêÙ?ï«­¡t•?ij×Ù(!?…—´¨?ij×Ù(!?ïì,´Š?mK/ˆ>·?cÓKÜjV7?mK/ˆ>·?êA>Â;,?ËþeMY?ÇÂû÷P?ËþeMY?ïê–ó]A?–ndØ3íŸ?Ÿ'­#L%ì?–ndØ3íŸ?ïuõÓx°?Ÿê8Á³+K?'MáN'ïø?Ÿê8Á³+KAGN3FGL J0725.7-0550@kÂW§†Â'@ªÄ°ž™À:&¸©õÀ;']<9A?çâÉ|œnò@äJ¾À¶?ý›ù?ò^W?êIHQŽ¤.?¢U'Õ«~¿¼Rk¡}'¿à)êÚ©Ú/UNASNone@³MZÀƒoPowerLawnone?ïþ¨|‹kÙ?!I/^?%x:ÓAÊ®?!I/^?ït'g'¥"? E ü—ô1?'o³c)®? E ü—ô1?ïÜCÀÒ¡+?m$ö' ?qÞ|'bÇ?m$ö' ?ïˆÎig?oÚSs¼˜?Ì_—ÿ¶e?oÚSs¼˜?ïúø8'ÊÂ?BzÔæy¤Ý?DÇð(?BzÔæy¤Ý?ìvŽ[fÇÏ?ÄYh`*{î?¼K$ÉÁˆ?ÄYh`*{î?ïÈÆ1Aq?}wù¸•?{œç}
ka?}wù¸•?îÑÞ5>M?<}zMOÉ?¢â³Gž-?<}zMOÉAGN3FGL J0725.8-3532@o`—ÌÀ"ôù;À À:zÑWv	À;qªt³0D?Ðx+úé@"9náŠ@ÞL€S¿éø$ÆLÄÄ¿æ7BÙ»À¿ãõr
É¿½céL&/UNASNone@–;ºÇË)PowerLawnone?ïþ¥íîc?2A,ßaó?/£5C±?2A,ßaó?ï£üTàé ?–ž"è¡Å?‡êÀæ€ ?–ž"è¡Å?ïÏto•Ü?o0j–úÀi?xEö4÷Aä?o0j–úÀi?ïë"cZ ?P¶ô—ž?d{œÌ[-?P¶ô—ž?ïõTÇ=ÒÛ?\œ­.#ºQ?UVq­•šŸ?\œ­.#ºQ?ìõwÊ֗@?¾‡È÷*Cu?¸TA§"x?¾‡È÷*Cu?ïúäY¨µ?"]òåÀX?œ £yòSR?"]òåÀX?îôÙ»jI?•´ëą«? ²dLÍçi?•´ëą«AGN3FGL J0725.8+0212@jÜÇ÷zö@@!U0H'ÄÀ9|DeNÀ;{àdYEì?Ä<fõÌ@õ½ê0àÉ@zDßØî¿å]àÛÍq¿â7ä¬M·¿âò|Ԛ¿ß8ÅJfUNASNone@˜%+ÓÃaPowerLawnone?ïþ.Øõ=ô?%)ì8Q	?-sÁ"Ɂ?%)ì8Q	?ïº?ˋÈå?ŽšªY¾û?p

—ˆÁ?ŽšªY¾û?ïØÜvIC§?z6ø!RÍ»?s'Äéœj?z6ø!RÍ»?ïåè›ÏÅ?M #nrjÞ?jd+hہ?M #nrjÞ?ïùôä ¯?B"?½—â@?H,o¸ê\?B"?½—â@?îG2Ò÷D?µ¿·ãO©?«ŒÒÍø÷?µ¿·ãO©?mPv¡?Ž…ß'˜?šdž#çÈ?Ž…ß'˜?îéAw$2?Žad¤ï?¡k苎 ç?Žad¤ïAGN3FGL J0731.7-1914c@mRd"¿Æ·\"?ÅéÀ9©ÌíƒüÀ:ì±+†–ˆ?í{‡¬ ÷ @Ȭêˆõ@+ÿwD¿â%q/(rÌ¿í_ÇÑÃà¿ãöÛ¯yç¿×g£àeUNASNone@ƒ
N¤¨ÁUPowerLawnone!?ïÜnQ}‡?t
˜HӄÕ?qòÈ´å$‡?t
˜HӄÕ?›âÒ¦?µ/Jä]jÈ?¥G6DfŠ™?µ/Jä]jÈ?îî…ú¼…?•Z̘À?¡ל䛮?•Z̘À?îï"㇬æ?ð¦gQp?¡±Èa¤?ð¦gQp?ï_íVbÀÈ?˜ùVq‡"?"U,ȯ?˜ùVq‡"?âCSJfç?Ð&œêåo9?ÛyYk3Þ2?Ð&œêåo9?ë&Û?'x?¯7¦¢{}?Ãg¬"¶?¯7¦¢{}?èÛbi£Ú?µ–0Z³!L?̒vYùpš?µ–0Z³!LAGN3FGL J0731.8-3010@n†!ê5"À˜¬}¡ìNÀ:|"}ÙI³À;ÛeìÃã¿Ö•´2Þ4å@ÆËG;¨Î?úµ1 6ç¿ïÿ(Ÿ˜??ïÿ#üY¾¿ÚÒÁb$Q2?ÇñÎ?yδUNASNone@Åk.—OßPowerLawnone?ïþ²0¥v?-ïÉB1?/Ù¤ÕùU?-ïÉB1?ï¬ú}¬v?'h´X³Ï?"ÿAgt"?'h´X³Ï?ïÐ8ӗR~?sç{зN?wã–'ø)5?sç{зN?ïþ˜1˜1?€®b3!?&|ê'wÄÚ?€®b3!?ïú (Ù+ð?I%Ê}©ÿ‡?G]B)?I%Ê}©ÿ‡?í±ÐKv9Ý?¾LˆLrÓ?²q}¤¼$˜?¾LˆLrÓ?ïº>ôBð?€.¼Û¯êò?pBÿGà?€.¼Û¯êò?ïò>!‰ù¥?W`¾U–'‰?[ƒ½#vY?W`¾U–'‰AGN3FGL J0733.3+5904@c¿")³ú@<O…ô¡'À9ûçéóNÀ;ùŸ¸—‹¢?¹Q¥mü÷@=X´ÌûÇ@>2ÿ±¦¿ê
π8ï¿ë†ØÕÕÆ,¿Ó½ïù'j»¿èúÖ0´åUNASNone@y™¡ ÏPowerLawnone?ïÿÀºUµ>þ""BÒ>ÿ£íc³®>þ""BÒ?ï×ޛ¬Cj?'óå}cQ5?t²Jڊ¡?'óå}cQ5?ïíCcƽ®?o§1½QV¢?b¼œÇò`?o§1½QV¢?ïòSFÎñj?@øº½8¶"?[Yqëêœ.?@øº½8¶"?ïÿÜéœÞ•>ñxœÁFÏ8>ñ‹Sd">ñxœÁFÏ8?ï
:¥Ý?¯mΛ¡4?ž^ø¤e&U?¯mΛ¡4?ïçrÀ-O?pŒ²{HèÖ?hé|KÑ?pŒ²{HèÖ?ï¬Q+¹
Ë?x(®s;#&?"ëµ¼\?x(®s;#&AGN3FGL J0737.8-8245@rq3|™®'À9t_ZÙjjÀ:
jÿR[À;§£@âH_¿ü5V¹u,'@
Üme35Œ?þµˆ€»®¿Ì4Xþ…Þ¿æ×(Œ¼¿Òð[Ç빿Åkí4²uoUNASNone@¯A"&Á¾PowerLawnone?ïþ_*vºá?(Åfª'CÀ?*
\ƒyg?(Åfª'CÀ?ïÏvߟ&:?ŒÀ¤Û…ç?xD_Ÿ?ŒÀ¤Û…ç?ïݨ|¶^÷?p6o¢(5?q+Á¢Ôk?p6o¢(5?ïÿûô`B>>¹ô¹#Ây>À.%»ï‰>¹ô¹#Ây?ïý š)ax?:€<í€
?6û/~*)µ?:€<í€
?ï-R>ބ?¯ÛI¶Y"C?š]u¿gg?¯ÛI¶Y"C?ïÙ$jSÂ?wÞ*Üç;?smÊÔ¿%k?wÞ*Üç;?ïÿÃWEU?¹óÈÙ$>þTŸÝ;?¹óÈÙ$AGN3FGL J0739.8+1312@iÊsÕº²@0Ÿ(bõ˜žÀ:+ÈbÚÀ«À;µ¢4rÎ?ôT&£,ëF@¶½[À›@àpÍ¥»¿ãGÀ-#œ	¿é+œÔóž¿ïÿÁÄ[D¿á<ƒbê·UNASNone@zù=ÙcPowerLawnone?ïÞÂ<?–;ø©Ÿv'?ŒºHMàý?–;ø©Ÿv'?ßæ8³Hº?Ò"@{!?àãø&[£?Ò"@{!?ín˜}KŽ?¢M!.æØ?´‹<ñ.?¢M!.æØ?ä‡6ܸ—?µ(…bÞz'?Öñ"þFŽÒ?µ(…bÞz'?ï8¢<?¨|""áä?ÿÿ˜ë¸?¨|""áä?º³ÑœGýM?Ä«Øî:¨?쩅ÌwV?Ä«Øî:¨?ëxˆ<ð?«ôòBÄ?­ߴB?«ôòBÄ?»×ÓPŸ¸?µšÜb1œ‡?ì…•ì	?µšÜb1œ‡MIXED3FGL J0740.6-5230@p'DЩ*À,…æÿ}úÀ9ՓW`9&À;k¶1€¿ù‹·Shݺ@õÔȧÏ@×ß?k$ç¿èÄéeM¦k¿ßÙØ
e,¿æÊ^Eäv¿ØŠ—È<UNASNone@™;©"áPowerLawnone?ïõ4¥N-µ?aÆåYñðì?U–µ«t½?aÆåYñðì?ïǟlÓy ?qåò?|0I¤±Ì&?qåò?ïŸ8–ÊÑ?~ÀÕk)‹?ˆ1ډ¦?~ÀÕk)‹?ïÿÓQm¨F>ñå"36éž>öWLˆÇ>ñå"36éž?ï·mŒöH?ˆhF½?'$œÏ$‡?ˆhF½?î¥j3ê,?³ŒWr\Ý´?¥©\ÄÌÚ+?³ŒWr\Ý´?œP6?ŸQ‡³ÈVâ?¦Xú†?ŸQ‡³ÈVâ?ïùŠä†8$?KÂã=5³¹?IÔmxv™?KÂã=5³¹AGN3FGL J0742.7-3110@nÆw[0À®S<½öpÀ9{lØÀ;Ød°ƒÁÀ0tY™#}@¯h¸Ñ@½üÂØØ¿à±s39¤x¿èê|ã!ð7¿ä¥ïÑ3º¿íŒì"Š³oUNASNone@•`åýŠÚºPowerLawnone?î')uÖW ?±…/­¬Eû?­hžO?±…/­¬Eû?ï¬Ê
G#"?–¼2µYʔ?"Í}q¦Ó—?–¼2µYʔ?ìø^'‰?£-óÈÙ?¸=œé?£-óÈÙ?ïÿç(؜>íõ‡÷>è×7Jˆ˜C>íõ‡÷?éþ‰½qÝ?Å?Œ)e÷M?ÈÚ
8‹?Å?Œ)e÷M?íßj§ÏÎp?½BDïÌ<?±ªÀ7²?½BDïÌ<?èîw‹
 
?³'¤•#§Ë?ÌF!ÓË×?³'¤•#§Ë?ïüFvÿ2G?AJföIö³?=ÌH¿%'é?AJföIö³AGN3FGL J0744.3+1715@i\í(Œç@3?¿¤Æ†À:0áþ99À;¼RÀ—4e?ìÝ$ݞÅí@šö†M@ៗµi¿ÓÝz:iïn¿âkዲ¿ê—Ž$"¿çAê%DªUNASNone@•ÑNV"PowerLawnone?ï…éGw?¦ÕމÒà?Ž…®8ÆR?¦ÕމÒà?ç×>
N??Ç;É7t"?ÐQ݃åcƒ?Ç;É7t"?îqX—ñ£Ç?™jÎ7ØtÑ?¨êv}v'™?™jÎ7ØtÑ?ç ³Ì=?¦ô–¤ÎJ?Ñý¾˜gч?¦ô–¤ÎJ?ël.kŘH?ÃX«»½Ì?ÂOFPéžâ?ÃX«»½Ì?È¡yñÍQ?ÇÐ}÷Jé?éסƒŒ«¹?ÇÐ}÷Jé?éha~#?´ƒ¯2Ä4?Ê_ö{®v?´ƒ¯2Ä4?À`aVS–"?ªÌû"ãÜ?ëççªkx?ªÌû"ãÜMIXED3FGL J0746.4-0225@k¯\(õÃ@&*¯È°À9¦´%6nÀ;'ø
h9¿Ç*G@C¬@]XXܐ@Eß³.k¿ã¦H®¼ä¿Þý´7÷àn¿àjê.÷(¿Ôá)E\UNASNone@¡¹Ž¤¨ÁUPowerLawnone?ïÿÈR$÷?·-•ºu?FøiyÝ?·-•ºu?ïÈÀŸS(,?Š1Ni‹)?{Ÿ°>^¥÷?Š1Ni‹)?ïèà"Âæ?lf
|)ùþ?g{½	Ù?lf
|)ùþ?ïüÓ¶S—4?#Èæè?9bN1û¨E?#Èæè?ïüĒX¹?6Ú¶Çü– ?9Ûn^g°ú?6Ú¶Çü– ?îÜG†Þ/?²I<ÖgX¾?¢;‡š²?²I<ÖgX¾?ïÎZ
	[?}€F¨ƒ0ê?xÒù_C†¹?}€F¨ƒ0ê?ïànX‰j3?b Òã"ô?o'§aø%h?b Òã"ôAGN3FGL J0747.4-0734@lF`ªdÂø@!£Ð|"µÝÀ9û™
þ`ÄÀ;wÖ	Œp¼?Ùý%	NÞ@fñ/
@笿'%¿ì+£3:Ê?©¸Á"bçº¿à›ƒ†²·"¿åë!²¾iïUNASNone@¥ªbMÒñªPowerLawnone?ïý=°ªX?COŽ½B¦?6},0Õ?COŽ½B¦?ïmɤ¤9±?™Çøzñ%?'FËnèeç?™Çøzñ%?ï׎÷vø?mlc5ól ?t8"CW«Ö?mlc5ól ?îÚìd.?€!DúU#"?¢Q9µV¯&?€!DúU#"?ïë!² ?f	Á¢?dàÞ«µ8¦?f	Á¢?颲UŽc?ǂd9̐£?Éu6©Æs¨?ǂd9̐£?ïwìyvŸ«?Œ½p^Bóž?'pØBŸ?Œ½p^Bóž?æÆð ™y?±¯7åšZ&?Òrð¾Í
?±¯7åšZ&AGN3FGL J0747.5-4927@plçl‹C–À'ÎÛ0sÀ9ÛS¸
øçÀ;k(zrŒå¿Ð=tÄfæƒ@
pó'ß@B@0þ'î¿ç$
Ù©Ì¿ènè\ ¿ÓÞ d×ú¿Ý¨-óòðUNASNone@žÍquŽPowerLawnone?ïýŠÜVFw?@Zr³Ò®?3©I?@Zr³Ò®?ï½îýƌ8?ÑA«ºç?€"@˜SÏÝ?ÑA«ºç?ïۃWý†Ã?j6šøê?r>T	'z?j6šøê?ïù®HÁÿƒ?2•ÐSô?IFÝM8C?2•ÐSô?ïñ®}KÊ?dÕb}ç¢?\£¢-T?dÕb}ç¢?î8²*#þ?·;¢Z—Ø?¬tÝY"M$?·;¢Z—Ø?ïlî¦nò°?'oŠBâR?'b+:¸°?'oŠBâR?ïȪ×b/©?o
†+š?{ª"Tg‹¬?o
†+šAGN3FGL J0748.7-5116@pˆ¥ÃÞç'À)1!îgQHÀ9Ê´øš°ñÀ;cÛêw¿¿áiô/3Á›@
ìŸÊ5BØ@÷L_ª	©¿Ù²öcm^¿ïs5Hم?ԡȕc1±¿æÇ"µ¦Y_UNASNone@…ïWÛô‡ýPowerLawnone?ïþ`L_ÃÏ?2àjžÄ*‹?)û;܍Q½?2àjžÄ*‹?ïÁ…JÏ~z?Žå@§‰?=Z¥ÿ2Å?Žå@§‰?ﯽ#{I?Ê©©S˜P?"·)Õß?Ê©©S˜P?ïý¤i'{ÿ?(¹©ƒ2?2ܱS<C?(¹©ƒ2?ïù´ùé²Ù?SǞp?I,æÛ6D?SǞp?îeÙG¤s?¶Ð	Jàº?©¢n·:5Ó?¶Ð	Jàº?Á¯/?"Ú¾dð"¨?œo̟32?"Ú¾dð"¨?ïö` Éd?U*îa6A¬?S?øJúY3?U*îa6A¬AGN3FGL J0748.8-2208@máî¢
?ý¸Ž¼ÆÅLÀ9z
>GclÀ;0¿ö$µ¿ÜÞQêƒl@
q†,ÕK!@ìÝÀ$5¿è»q§{ô1¿é
!þÑ$¿Ø'ç5¦"¿ç†Ú6(UNASNone@'o§æšÔPowerLawnone?ïîbþ@Ññ?ƒ*u.&?a²Ïvþ?ƒ*u.&?ïíO½ò-? 0Zܸ?ˆ"¬4 ¼? 0Zܸ?ïŸÏ¸(iÅ?ƒ)ôÒƨ?ˆüÄÆ ?ƒ)ôÒƨ?ïôä‰é©?COMrAª?V6ëظ^È?COMrAª?ïϘVxÄ?{r‹ui?x3±rPAó?{r‹ui?íf\ë¡?½~ö2ÕGù?´Íˆ$‰õ?½~ö2ÕGù?t ?œÚøšÂÚ?¥^{"@þ?œÚøšÂÚ?ïy.é¦w?ƒn÷(pڄ?Ú=4+"?ƒn÷(pڄAGN3FGL J0749.0+4459@eÇ;÷'j@<ž†"ÄPÀ9áÀ¾¡ßÀ;âïÙAOV¿æ ž†~@KÃ Ô ~@ùY_í¦a¿æîÜü'.¹¿â^Ø܋ÂÓ¿â&(¦I€¿ëBýùóÿõUNASNone@‹%µ¨Xy>PowerLawnone?ï÷¤as¸_?SÂÞH_"4?P·=~C²q?SÂÞH_"4?ïۄÈÒc?'‹À$®¼?r=›¨"ڇ?'‹À$®¼?ï©·÷}¥r?#=Æ?…'*åwb?#=Æ?ïýâq­J?2¸
úœ?0ìt™[©ã?2¸
úœ?ïêdwC?fk8G™–?e›äŠ:×?fk8G™–?ï,àÁ q:?®/C¢\¯Û?šcçâÑÁ?®/C¢\¯Û?ïšìCÏQ?˜HvV³?Ÿì¢tyÕ?˜HvV³?ïã3¶»¾]?c²"ű^_?lÌI/£û€?c²"ű^_AGN3FGL J0749.5+1320@iç×Ûôˆ@2Ññ{ؾsÀ9ñªÖÿµÀ;Ÿ»@³Nw?éÀž‡§ @ºd>@þ–Ÿ¿"•¿í¿úÙ{?¢Þ,1¿æãtS¹æk¿èfžàs¯UNASNone@™V?PowerLawnone?ïôøZDD(?Z¤gÂ?VK'M?Z¤gÂ?î¿«X«4C?¦mÁt`o?¤JqÝÓ?¦mÁt`o?ïs"·<ö?ˆéÐP«bF?'Ÿia:?ˆéÐP«bF?션¹Ûêˆ?"€
™'ó?»Ó:1 «¿?"€
™'ó?ï€Bû¨,"?"?!<¶u»?ïA C²Ö?"?!<¶u»?å(šË?P?ÌEwrA*?ÕÑ®Êi_?ÌEwrA*?íMocSü?¨£Ì`[Ù?µ""çí+?¨£Ì`[Ù?ڕnçš??±pnFƒÌ?âµH÷2á?±pnFƒÌMIXED3FGL J0751.7-2944@n½ºˆ&ª¿÷‹?cÃÀ9u°}á­/À;Ù|¸[¿Í_:û ¾@¦H<Ú¦Õ@šÿà iB¿ÚÎmÝdZÚ¿énÞov¿ïÿç
)"f?ïþ¹ç܌UNASNone@Ž6û_ïJPowerLawnone?ïúTÒ6»u?S+ހØpX?F¬¸	89`?S+ހØpX?ï$ìƬ?œ$)VÅÇe?ˆ¶üDÎTü?œ$)VÅÇe?ïF,iëV%?ÛË>î's?—:rǼ¥_?ÛË>î's?ïÿèìÏ1è>êå¸)6‡>çj=¤{Ó>êå¸)6‡?ïÏäq"&Á?"p'Ë_ˆ}?x
Ç!çÎ?"p'Ë_ˆ}?íGj#_V?Áð¼P?µÇ®wÓ?Áð¼P?ìùlþä¥?ªÇ:³!ƒr?¸4˜ÜÜ?ªÇ:³!ƒr?ïüے"ÉË?HDOùӟ?9#k"lº?HDOùӟAGN3FGL J0752.6-1629@mSýÉÄڐ@ôë?{@À9ÍRÿ" À;~%AØèd?ÝâDæ@
꟏&y@˜ÿ•!¿æÜ3"yl¿Ú ÎçG¿âm¡UrÅ¿çj;Çù ¸UNASNone@èé^ž	PowerLawnone?ïú:\ƒtÐ?PªÅ]¼!›?GŽ7q«N?PªÅ]¼!›?ïi¤€Ê¸?šá½ÒÒÙ?'Ëoã9a%?šá½ÒÒÙ?ïÕÐ4=ýÅ?oúdÔа<?uåÌcu?oúdÔа<?ïwìJÁo?w²ŸL¨y'?Ÿqzn?w²ŸL¨y'?ïÉj‹IR?~Êäóà?{J±[W–¡?~Êäóà?é V¨
ÿ?Ljÿ]â?Ë~¥_Ô«?Ljÿ]â?ï9¥ß³?–jû}b¡ù?œxËaËs?–jû}b¡ù?ç"ÌÏÀ¶Ù?­HG3ïf?ÐÖf`~'O?­HG3ïfAGN3FGL J0755.2-2633@ns-8Go*?ë©÷À9.wAýÀ;.ˆcp'?â)¾Fïu@(ä±ÅàJ@ÕÍØã\¿åÕIJ̬ì¿ç¯ ùN#é¿ë°ƒëÔÇ¿å['²ãÉUNASNone@~œºÜ	PowerLawnone?ïöˆ'Ôy?XuÇÍ`?RîÞÐ.d?XuÇÍ`?ïUrçíÔ?±û°	ÿ?œÕQ¡Jwy?±û°	ÿ?ïg'zï	Ž?ŒcHøâíZ?"°ªµÔ@?ŒcHøâíZ?ïœÆ}Zý?yˆâ܉&?œg,å_?yˆâ܉&?ïXÚåÇÎ?™t9Éáq0?"ä£G=¡?™t9Éáq0?ænõ]ƒƒ?Êñ½V&.?Ó"ÑDøû?Êñ½V&.?ìÉjWÀ8ó?«"i'í´
?¹´­Aþ8f?«"i'í´
?æàú?µØWNÙG?Ò?Ûÿû?µØWNÙGAGN3FGL J0757.5-0536@l6BB…@'õŒÒ
ú/À9Á‡ŸœÀ;•úœé°2?ð»¼x@dV7o-	@LÀM£¿äECÃ'º¿él~_½'¿ìf;}{ù¿ïÿhÅ*/îUNASNone@}GN;Í5¨PowerLawnone?êH‰»Cý?бò$Žï`?ÆÝÙð…?бò$Žï`?Ê	iÖ]oG?ÈiA!³Y?é}¥Šh¤.?ÈiA!³Y?ë÷–¸ÏÐô?§)¯2Õa¾?À!¥À¼/?§)¯2Õa¾?Ø|BßVDä?¨X°'xv?ãÁސTݎ?¨X°'xv?è¾é¥©%?É5õ…Rº¸?ÍYi[kê?É5õ…Rº¸?ª½
Â8º«?¾O¹f=¡¡?îT/S÷ñ5?¾O¹f=¡¡?å .­"ɕ?¸ÊŽ'Ð7ë?Õ¿¢¥ºlÖ?¸ÊŽ'Ð7ë?¦Éë·lÀ?ƒ³eqŸ?ïÉ°°
?ƒ³eqŸMIXED3FGL J0800.6-4806@pk"¦óõÀ"·öµšÀ9¤ØDЩÀ;^
œ;4‰¿æu«'	@fÚÄT®@|ž_Ñ÷¯¿êˆ5Nt	ñ¿æ"Hô‹¿èb"ˆª"¿ïÿ˜ÞL•ÊUNASNone@€øØbMÓPowerLawnone	?ïåAÚ?oèËO?j¾a÷*<>?oèËO?ï¶!gXÔ­?LFl°^U?'w¦4ɔ–?LFl°^U?îúžˆ°'?o_ã}Y? Vt÷ßÜ?o_ã}Y?ïõö¡SïŽ?BÝ5¨¾*?T¼ê-e&?BÝ5¨¾*?ïÛÁgz?vÉ ¯rÕÓ?r@.a8?vÉ ¯rÕÓ?íß2F'û4?º/G5?±mÊKä?º/G5?í¦º£nHw?£àpVtîÏ?²Ê*åi£H?£àpVtîÏ?ï&ÅÓ£<?–èø!†?›']¾¬`Œ?–èø!†AGN3FGL J0802.3-5610@pÞ䣃'gÀ*YÛ©¢fÀ9ÏCŸ'À;w|ÚQ?ô —•Ž•@VϺ½Ö@í a´Ñ¿æ]†,n6Ù¿â:½h€Çç¿ë–‹¥|§¿îÝЮaZlUNASNone@ƒ,záG®PowerLawnone?·äAýx?¶³Ù;ê¸?íÃls=1?¶³Ù;ê¸?À¼¦…?ÅojµšE?ëøPÖ~ž¹?ÅojµšE?䆆›©Øñ?³¸­Â+Å<?ÖòòȬN?³¸­Â+Å<?ÐÅ¿"¦YW?¤Ya?ç n¬ÓU?¤Ya?ƒ-àHŒ¯#?Š´šb†!?ï³HÅÃ?Š´šb†!?Ÿ­®¼zöê?´]Kk="©?ï'ŠiÙ?´]Kk="©?Ç_
Q'š?±'›ë.?ê>è=k›Z?±'›ë.?•6‹ó·Éæ?}£Mª´EV?ïVK +Gñ?}£Mª´EVMIXED3FGL J0802.3-0941@l½XdE#ö@%òéhSÀ9ŸúE«Û»À;ŽŸ±m¿ð·¹Ù&w@¤gÕ&b•@A¦`|l¿äÅMíHÃ=¿âøœ×Å+÷¿àРÖÇû¿ß×çõ"ŽUNASNone@"'"h	ԕPowerLawnone?ïéH³D‡ç?¦àLœ?f·Lú°èò?¦àLœ?ïËcÏû©?‰'j2?zN[%s?‰'j2?ﺺG}ܾ?|lõì<¾÷?Qn àÆb?|lõì<¾÷?ïþU=Óu?viÅo?*®/Wÿ?viÅo?ïã0Z!ç?pë\ËDè?lÏ¥ÏÇÐÒ?pë\ËDè?îéÑo@L?±î'x¦ì?¡béû>ƒ?±î'x¦ì?îφC· ý?œ¸çw#÷!?£›Áò;7?œ¸çw#÷!?ïÚKª<Bë?n+"Ón>?rÚ*À2^œ?n+"Ón>AGN3FGL J0810.5-5214@p±´êJŒÀ$L`Ÿ±À9NeÜÓ«
À;E"äE?Ù¹e'è
Ò@\¬ 7@f"_ ¤{¿æÃǞ`¿êÖ!"VˆÅ¿Ý•ôgµ4Ä¿çø¡¨ör§UNASNone@"J1ŸŒ¨PowerLawnone?ïü©	ŠS'?:#§ù°AÆ?:·´å¦W?:#§ù°AÆ?éKÍM?˜j÷í"\ë?ŽÜźË½?˜j÷í"\ë?ï҆õtƒ,?pƒ£<ˆ?v¼…'Ú!?pƒ£<ˆ?ï{{L³n?m®³1EG]?–spüG?m®³1EG]?ïõ"…ª¾?W¦6h¥c…?Uºô1'"º?W¦6h¥c…?êóo›:ÐÙ?ÁUKa¶˜?Ä2A"¼?ÁUKa¶˜?îèÍCºÁ?›»óý:?¡s+ÊøÐû?›»óý:?ì¾´S??£0ôÅË?¿
Z]f?£0ôÅËAGN3FGL J0813.5-0356@lG
Ø/×^@0C#À:ZPÀ;µ©FµÆ÷?æ4ô9´h@ÁìóˆÎE?ú¬_©÷¿ïû^Õ¸?ï­Z®CÂ?•ÉæÁ7¿ÖIWé9ÚUNASNone@¸ã?PowerLawnone?ïþJ\ÏÂ?,¥ýNØY•?+_÷sSޞ?,¥ýNØY•?ï•ÐÜÑқ?'Õx~'3‡?Š‹ÈÙIÉ'?'Õx~'3‡?ïÔK—`·Ù?kÐƼEuÀ?uÚ4QëT?kÐƼEuÀ?ïT¸'"Æ?{3ƒ íûŽ?•hûÀY?{3ƒ íûŽ?ïø'êšß?M5ǵ¨BP?M´UÕT®[?M5ǵ¨BP?ìÚ?Ĝý?Á%׌æ¥2?¹.:¶ÿ?Á%׌æ¥2?ï¬Îq´ð…?:ö¥~R?"Ìc™£Õ?:ö¥~R?í¶ö
ÖA?£kàqñê&?²HO¨ƒ}?£kàqñê&AGN3FGL J0816.1-5044@p¤´êJŒÀ!9¨Íê>À9«aB:7À;#þT.U~?ôŸY÷î
º@=FŸ¡›q@òÙ æ[¿á‰3hH¿çNM;®=&¿é
ÂØŒ[¿í'íõUFUNASNone@ˆð#̎PowerLawnone?Ö®aÃ?Ç(½lMd?ä¨Ïrwx?Ç(½lMd?ÅíÍSìws?ĕU~Ùò?ꄌ«â#?ĕU~Ùò?çêq«hùê?¯T•ù9ø?Ð+©.-?¯T•ù9ø?ÚÉr¦KêË?¦*—Û¤7?â›F¬Ú
š?¦*—Û¤7?¹†¨.RÖ?¹ŸýÇý–T?ìÏ*úClU?¹ŸýÇý–T?Ÿ¯"¹¨0J?´Wä×?ïƒZ	ƒ.?´Wä×?Û7;¹r/¦?·†‡EPŽ…?âdb#Fè-?·†‡EPŽ…?¬)±òY?»Í•€õ?î>/ÝW"j?»Í•€õMIXED3FGL J0818.0+3237@g²(¡ß¹9@?WG²JÀ:8CÔk&ÀÀ;çÖNUο©¢ñ^¶öu@!¹f"‡Ý@q]À¥w?ç:¡f—Ž§¿é©a¿Õ$¾í!g?¿èaFNm÷)UNASNone@–šð ě¦PowerLawnone?ïÿb†\ûÙ?m(ìê?¯3Ô8›	?m(ìê?ïØ9pd?ƒ`ÃMíÕ£?sþcP¼ðß?ƒ`ÃMíÕ£?ïä2ѹq?hè͑GUt?kçÍp??hè͑GUt?ïð±íùB?E¨W/ð?_Ԝ‡:ß?E¨W/ð?ïÿ'BˆÙ?/.C-¯?¯RÿPz?/.C-¯?ïߣê?­$5÷¹?œŸäª*?­$5÷¹?ïß»`''?vRzÿ®)&?p"OÖÅ°?vRzÿ®)&?ï›fyöTõ?{F]æôÃò?‰&a~û&µ?{F]æôÃòAGN3FGL J0823.3-4205c@p<†DR?hÀâøæ0K!À9‹j˜û)À:»Þzt¿ñŽ;AŸˆ@NûÆ_u[@~µÀ@ÍP¿èBS¿âÕ­›rü¿æ¹Lé×cm¿Ðõ›Ã?…QUNASNone@¸‡"£S&PowerLawnone ?ïø£€Å…?YÍ|˱²~?OrQ"€$?YÍ|˱²~?ï¤	hDÉ?˜³ú
?†ý¥ÝŸ­Û?˜³ú
?ï	>4:'™?•ä—/6Bj?žØ9pÆô?•ä—/6Bj?ïÿÛæMÚÝ>êRΦ­&>òȉã|A>êRΦ­&?ﶀ.&Y?†²Ü¥v¶Z?'_ÜÂ4Ù¬?†²Ü¥v¶Z?íl¥W'ãó?ÀB¾+I?´šÕCÖÓé?ÀB¾+I?íQS£Qdˆ?§vï:-?µubä˜ôÃ?§vï:-?ïýXЎ?4°TËôTÝ?59䑽•?4°TËôTÝAGN3FGL J0823.6-4838@p"HýŸÓoÀ´]+TBÀ8ö$"]?vÀ:ó¸°¶Ñ?õAš	.Ï@þdRåÖ@æW_¸Lb¿à«l	¾o½¿ëÝüÓm®¿è8¢ÆœS¿íOÂNÞNUNASNone@"X'»0PowerLawnone?ïá{¶bZÇ?iÓ\7~;ƒ?n"IZLáµ?iÓ\7~;ƒ?ì''™¢Ô?¸Ô¡Å߉?¾Ã{ë2éa?¸Ô¡Å߉?íý…hxÿ	?å"¦WŸ?°Ô½î¶?å"¦WŸ?ë‡y_×ò?˜U¹úÚt?Á‣˜:?˜U¹úÚt?ï²îB­?‹ $¦' `?ƒz"l•a?‹ $¦' `?Ö­ëñ*O4?Ë̺¡Yµ?ä©
jØf?Ë̺¡Yµ?ìЕþžDé?§[c|Få?¹{PW³7?§[c|Få?ßÔ4ßt‰?µÝҋÄ?àåE»?µÝҋÄMIXED3FGL J0826.3-5056@pµìß&k¥À…ñ¾ôœõÀ9C¾b¦¾EÀ;*Aç+ä?ð¥YEÁ€=@a…'ͼ@ÓÖÀk•z¿æo0m
Ó¿È©ü¯#Õ®¿á¡Ôñα¿ïþCj–fUNASNone@šhÁTɆPowerLawnone?ڏ©2`Fß?Ïß¡ùíõÅ?â¸+fÏܐ?Ïß¡ùíõÅ?äPªÎ†r?Ǜ®3{úÅ?×ó^ªbó?Ǜ®3{úÅ?åq¬«5x?³=¸Q:'>?Õ§ö©•?³=¸Q:'>?æzwYA©‡?¤Î›«ƒD?ÓM|¬ñ?¤Î›«ƒD?Ã"uo\ÿ?Ï/ŽÊú?ë7b¤(؀?Ï/ŽÊú?Â68ÀÞN?€\NèùÝ?ërqúÈl?€\NèùÝ?Îâ!âlµû?º;;n¯ÏÖ?èGw‡dҁ?º;;n¯ÏÖ?ÍöƔéƒ?°™ú­ÿ¯?è'NZŸ?°™ú­ÿ¯MIXED3FGL J0826.3-6400@qfþ=ÁÀ-L4"…ƒÀ9õVI¸±À;­i#L5¿÷'Ìg¢%¯@…×Sƒ¶@¼tÿ[j_¿èš¨
ܹ¿âs? (ÿÔ¿ê#2X(c¿Òpå;¿¯êUNASNone@'!–R½<PowerLawnone?ïô¸–+rl?aFÔ"Ë?VŽÓK¥È?aFÔ"Ë?ïÆp<܇Þ?¹=if!Ò?|ÇátßXö?¹=if!Ò?ï"8\Îô+?'ÙÆPÍö?ŽñèÚeF?'ÙÆPÍö?ïÿ¹ãTèS>ûl}
^f?‡:³É"Ò>ûl}
^f?ïi<GÙÞ?–äo*Û÷?'ݘuLö7?–äo*Û÷?^P‡?´RÙePU?¦Æê‹CO?´RÙePU?íàþ7}ðœ?¢':ãRa?°øD~n¢?¢':ãRa?ïó‡ñ*Ù?[µñvå[?XñÈx_þ9?[µñvå[AGN3FGL J0829.8-5239@pіœ#·•ÀªB9`tÀ9rƔ¤gSÀ;:?wTW?×Ú+´RœI@
€ˆ!ö@}úÿåþÍ¿åöR­!¿ë½²8Ýþ4¿â5Ài;'¿èiÕ°ïUNASNone@†#·€4mÆPowerLawnone?ïópúWä1?c2
E/?YŒ°¼ô?c2
E/?ïOmQ֞?žœî9ŽT?–UÙU8?žœî9ŽT?«|¬4?'\¢%Úß"?ˆßUõºü?'\¢%Úß"?︨ã?zR?ðc#?ˆýì´±"?zR?ðc#?ïÃ()Œ†?ƒTp[»õ0?~këfºüð?ƒTp[»õ0?æ^µ¸¼¨?Ëñƒ-¥j?ÓB"Ž†¯Ì?Ëñƒ-¥j?íß.Â=Û5?¤÷î–N ?±‰í£2Õ?¤÷î–N ?粫pS¨?°¦ßBê7 ?К©Yȯ?°¦ßBê7 AGN3FGL J0830.5-4452@plÎp:ûÀ
Nb®•ªÀ9ò"Ýr6À:0‰ÁµA–¿ãö¸%^
@‰ÿÈ¢œ?ÿ9{ßto>¿éP¥:üD#?ï½jòŸd?Óa°¦Ûj¿èF¶]I²&UNASNone@Çß#t¼jPowerLawnone?êÊ#Ê,?ÊgŠÕÓÓõ?Ä×p×Oÿê?ÊgŠÕÓÓõ?ïŸ9"kúq?˜¨Þ`<
Ÿ?ˆ1›!'Ç©?˜¨Þ`<
Ÿ?ç휻• ?³'Ûã¼…?Ð%þƈԿ?³'Ûã¼…?ïþ0‰#™|?1YQEú"?,÷j¹Á'?1YQEú"?鬲.L)à?ÉšR|#½?ÉM7FÏX?ÉšR|#½?í3K²c'?Án·á¶ÇZ?¶e¢n,íð?Án·á¶ÇZ?ê¶ä â‰ß?°ÂTZ«?Å$o|u؅?°ÂTZ«?ïúê÷|›)?NʝY""?DT!)mO?NʝY""AGN3FGL J0830.8+2629@h­>À//˜@@F¾œˆacÀ:-Ü^:GúÀ;Ê zÉʺ¿ÒŽAX²@&@HNx^@tPÿ÷Çw¿ækš
+í¿é*l{¥¿ÜrWÙcg¿ïÿᘴ(UNASNone@†àÞ҈ÎPowerLawnone?ïþìzù+·?!¯L½ž?!8RL§¬Ë?!¯L½ž?ïØ÷D'÷±?'þû–4o~?s"]ÑÑL?'þû–4o~?À¨YÙ?wÉõ½?ŠÐÕ鉥?wÉõ½?ïïCÐlòû?H­êé0 /?`¼/žÄÞ?H­êé0 /?ïÿKЖŽ€?!!%Šu'?…ëñþ%?!!%Šu'?ï<=6Ü?«ê¸c°À?œ~xzò~?«ê¸c°À?ï€þêE"?‹Ü—Réó(?ÀEn¸ß?‹Ü—Réó(?ïAàÆ1…½?Œ~žfiÚ?—Ãç18Bx?Œ~žfiÚAGN3FGL J0832.8-4321@p]1¤½º
ÀzMÙ§¦£À8ßÕùµcÀ:p•âTô?çžR@i§Ž@¾½Òß@`•ì翌»Ë'%Þ¿êFÑËå¿éô{Kû¬¿ØBR'X"¦UNASNone@¦Œ~($PowerLawnone?uëЯ?­å.)ŸeÕ?¤•h£Öª?­å.)ŸeÕ?ïîð¹,?¯
V¯´ð?œ"!èÝúr?¯
V¯´ð?é…ÛâœöN?³ƒ	?ÉèuŒ&È?³ƒ	?ï`äØ
¯?yÑÊpãØ?"ãpþJ&?yÑÊpãØ?ã%zI-ª?ϺF,µÊ?Ùµm¤ü­?ϺF,µÊ?ç,!ùúØN?ÊjÝÍÛ/?ѧ¼
Od?ÊjÝÍÛ/?âoæSå?ÀŒ(^_?Úå 3YÒ7?ÀŒ(^_?êhsíô â?µ¸Ø{¼í?Æ^0H-|v?µ¸Ø{¼íAGN3FGL J0834.5-4825@p¡JB®Ñ9ÀV¿2/'À9hhó ¸À:Äþí±Hã¿Âï÷<j
@Áe¥÷ @€w´—¿çŸÊR@Œ¿ê¤€HBl•¿ÞŠz܃èÇ¿êl¹oUUNASNone@œ_òa|ÚPowerLawnone?ïáº-ŸÐ?˜¾Ñ4ÜÓ?nEÒB½ŸÊ?˜¾Ñ4ÜÓ?ï™Q
q?›WgJ0¬?‰«¼¬¥,M?›WgJ0¬?î'åa‡ô?}†ÑR<?§Ñ©ç€¾h?}†ÑR<?ïó¥UÜÍÃ?B ZHÏY?XµSö­‰ü?B ZHÏY?︅±ÊÙ?€¡%)/N?Þ"†ø‡²?€¡%)/N?í%y·þ?ÀbÜÄ»?¶Ô7‡"@?ÀbÜÄ»?ìºù\$Î?©@¸ònTÄ?º(5¾Ù'?©@¸ònTÄ?ï"ÐÆØ×?|Å.ê3?‹Îx.Z?|Å.ê3AGN3FGL J0834.6+6101@cpŠGìþ›@AõÑN;Í6À:'dgˆ¥VÀ<
n.±Ä3?Ғf)T¸@Ëg!wI
@S;ÝÛ¾¿ÝpÑF⛿äpÓàx"¿ê'ÃC-ž–¿ãM®23ËUNASNone@Œ.$¨ÁTÊPowerLawnone?ïìm]óȇ?'j"_S?c'¡å»Ù§?'j"_S?Üç"?‡¤¿RëÔ2?€Èê09?‡¤¿RëÔ2?îè›Y"£
?—¾øº®÷?¡vJdF3h?—¾øº®÷?ï$¿kÔÿ?'`nL=`?Ûh͒ ?'`nL=`?ïžè…\m6?'(¢nQÕ?ˆEޛ&B§?'(¢nQÕ?ë°H'jü"?ÂÉæ!¡T=?Á>ݶTw?ÂÉæ!¡T=?ì%,—o?±p
"˜L?¾×ŸÓD‹?±p
"˜L?ã4e9›…?Á†ÝAd?ٗ5øÈö?Á†ÝAdAGN3FGL J0838.8-2829@oS\gßã*@4~êÁªÀ9©Û0=À;r-͘¤§?òMÂÎq<®@â†óNÂ@ÌÞࠔ5¿àth‡©¿àƒ÷à"¿äŒÌV°;¿îG\sQUNASNone@'';˜Çâ'PowerLawnone?Ä å´f=?Á'ßµôˆ?ê×ƺRæq?Á'ßµôˆ?Ê¥ T[?Ç$—.Z[k?éV—êþø)?Ç$—.Z[k?ãÏ­ºÚõ?´,WÂΆ?Ø`¤ŠäJ?´,WÂΆ?Ûp9š?¤yÎ; J?âGóúc3?¤yÎ; J?›ÑŠø"? Ï¶'÷ߍ?ï!sŒ¾"? Ï¶'÷ߍ?¦F6 D?´{@dµf?œ£º/?´{@dµf?ÂÂtRÑøÊ?²‹	¨E:?ëObëKÍ?²‹	¨E:?­¥[È ?ŠÇÙ©¦?î%ªPúÞ?ŠÇÙ©¦MIXED3FGL J0838.9-4056c@pI*â—9m?Ó@¦¹<ÍÀ8Ð/9©núÀ:mSB3'?Ä\G‹|Aç@Ù@ºZYh@MüŸù/+¿ç×{ÉÇV¿é' ÚE¿ë³3§*¿æâÓUÁÂFUNASNone@ƒCZA_EáPowerLawnone(?ï~+ö9=õ?˜ÁÑZË߄?:=ÿ«L?˜ÁÑZË߄?ïeÀÜY?«ß@Íè)?"^‡é¦žÑ?«ß@Íè)?êGÌcÒ?±»å¯5?Æã°Îp·?±»å¯5?ïÊùFŽ•ì?`}Ž#µI?zƒ\Ÿ÷ÚR?`}Ž#µI?ëgÂ'hŠê?Àîæ¡£íõ?Â`÷b]ÔX?Àîæ¡£íõ?ëOy}†9?Äñ*O3ïÇ?™ç?Äñ*O3ïÇ?æcE(?¹T|n"î?Ó9uÕͯÿ?¹T|n"î?íRÉ?hd‡?¡SŠh9ªe?µi¶˜ÂÅ?¡SŠh9ªeAGN3FGL J0843.4+6713@by•$Ý@A͂¡ ÏÀ9¦sŠ;WÅÀ;Βßk5?çÌ'æs@uÞ©n#?ÿàß=Ù¿æÑ´¬ß5¿Ü¬È$òRÿҜz¿;Ù¿ìº9$
üBUNASNone@ þô¼j~úPowerLawnone?îɏ­4?žª™´+7?£nWá¾?žª™´+7?ï†5‰Ø9?Xµnyj?ŽrÐñj?Xµnyj?éøi+—;?¯$Fmc
?ÈYûQ£?¯$Fmc
?íë´À«E,?%l«aß?°¢Yú¥Öœ?%l«aß?ìwý—ðÍ?´Úm,Þm?¼@@y—Ç?´Úm,Þm?ì	•€r?¾Í‡z殩?¿ÿ³SÿÜo?¾Í‡z殩?é´ž÷õ?±ëËê1‰%?É/§å" -?±ëËê1‰%?åýWÍ,ª?»ÔŠ¾+ì?ÔßPe¦¬?»ÔŠ¾+ìAGN3FGL J0844.3-4741@p§Î_oÒÀ¯ŠúšeqÀ9
£oÜ0îÀ:œÖÒ	L°?ì%p|ê·@H©}è88@±>ÿo6o?ïÿ¡"uÿr¿æ%ºÃϑè¿çŸd}G¿ìZíß
Ž€UNASNone@˜w©ûçl‹PowerLawnone?çäny&ÔÍ?ЗD•0SZ?Ð7#
²Ve?ЗD•0SZ?ìÑq)ìk?¾­crb•n?¿Ytv°œ§?¾­crb•n?㴔aêO?µê0º çp?ؖ×=Ð+b?µê0º çp?ëÍ×Ùñ"˜?žÊvz=…]?ÀÈ ˜;u¢?žÊvz=…]?ã·Yºþ»?ÕìÆv`HY?ؑLŠ‰?ÕìÆv`HY?Ûe7:1‡À?ÌV:KwÅ?âMdbç< ?ÌV:KwÅ?Ö´ïÚÓ?»1óm"?䥈x'–y?»1óm"?ß•òƳ?µæÀœpl,?àq5œý&?µæÀœpl,MIXED3FGL J0846.8-2638@oFÅCk›@$ªkøvžÃÀ:–ç7²À;œ}>ïÿØ?˜ÌÖõÕ@Ð3f´¿æ@ÈX *,y¿Ý´…XDοëX
Ò?l@¿ïÿ™]-š?ïü…û4Ç»UNASNone@ˆ¬o4Ö¡bPowerLawnone?ïý²J
?<žaâHhè?2m¯±Fº°?<žaâHhè?ïÁT¾É(þ?ŽŒ)ûnNQ?U "Ü\â?ŽŒ)ûnNQ?ïc¿íb»Ù?‡ït.µ{÷?"ˆLÉLß?‡ït.µ{÷?ïÿl4Á
?ŌíD?yPªˆ£?ŌíD?ïè€ãGì?pÌÓÕ@	?gÉñòg?pÌÓÕ@	?î¹e±à?³V–÷"%Û?¤nY¨Q"'?³V–÷"%Û?íZ‡€<{[?ªV¸ôRÍ­?µ+Ãþ%%?ªV¸ôRÍ­?ïãmt™ý?||ó/\ðä?lú'‹fÇ?||ó/\ðäAGN3FGL J0847.2-6936@qÆð:û~'À0@ ÇÀ:Å~#òNÀ;¹ë˕•(¿õ¾"_¦XÅ@™ýAµ@4÷ 2z|¿êu)6Òqt¿äëE
¡¿¿ë	õûÖ`Û?±zG(ÒiìUNASNone@‡ÑŒL˜_PowerLawnone	?ïýí+'n??4j²©í¾D?0–£K¾wq?4j²©í¾D?ïÇNµ½+?¢É9WU?|X¥&ûJn?¢É9WU?ﭐÂ?yOcøÈ]?"›ßÃ?Gx?yOcøÈ]?ïÿö—˜ÚÏ>ÎPÖº¹@>ÒѤ`æ>ÎPÖº¹@?ïøðÃ÷ç?QuëÀ1 È?MÈ=@ðÍ"?QuëÀ1 È?L"?´VôÀà+?¥‡ÞWÏúÉ?´VôÀà+?ïBí¶??ëYZc?—¼'B^ &?ëYZc?ïþÊì€yì?&§ý<?SÀ?#Q5:ä>'?&§ý<?SÀAGN3FGL J0848.2-4524@p'3]$žE¿ò.Ñõ*¹èÀ8Z¥öŸ..À:AJFu/W?Ü[wµn6i@*°ÁÔKF@:3q¿ãΞÜØ¿è‡Î¥%O¿çÚ¸'›¿æðu̓tšUNASNone@'œØâe,PowerLawnone?è6§qsŠ¼?ÏõŠƒÀÙ?Ï%b:1Õ?ÏõŠƒÀÙ?ïB]G®ÀG?¬…">?—´W?¬…">?å89Wd•×?¼¯Ðt™|`?ՏQ6ÔR?¼¯Ðt™|`?ïy¬O?pÆí;ä{û?Êv"Ÿ{×?pÆí;ä{û?ÙZµÞs¾>?Òg•¥ïr?ãR¥Æ á?Òg•¥ïr?é6Ä "Z?Çnk:&Ã?Ë$íõ®˜?Çnk:&Ã?áŸÛ}Ò?ÀȈœ"–m?ÝÄÀIØ\?ÀȈœ"–m?ëN™Á˜Í?¤ž0;¸ç?Âǹ˜ùœË?¤ž0;¸çMIXED3FGL J0848.5+7018@brGE8ï@A•"Ý—ö+À:€€VÒt¬À<i[
lÐÀ‰©6šœ@ýïÀí›y@eÀy,g?ÏM¤È½|¿å[¦‡ÙL¿Ö0«±LO¿ãl¥‹«UNASNone@¬q"!-wPowerLawnone?ïÿØÔ© ?Öv"çâ?‰È~´Wæ?Öv"çâ?ïàœwfá-?'8À¯ÀÉö?ocˆ­¼zë?'8À¯ÀÉö?ïë-Õ?fxò|)1?dÒàNí"?fxò|)1?ïÿþÍûËé>¡m'Ž†GÇ>£$ßÕP>¡m'Ž†GÇ?ïÿÂÑSø®>û‡j@sòú>þ—ko$é$>û‡j@sòú?ïI«foä?ª³M);~)?–Ê",Z5‡?ª³M);~)?ïëÁ¹À¢ê?iàýèp?d>FQ;
 ?iàýèp?ïÿæ˜áôã>ñÀL̽ïœ>ég3x)X>ñÀL̽ïœAGN3FGL J0854.4-4404@pŒîËûµ?âRuÚÀ8"­¨DWHÀ:DUFƒr?êOI£Ú\¥@¤'šG@Íù ?{¿âªÙ-5ö»¿ê"¶Êh*¿ëÅýÅ_'"¿×1¼áUNASNone@²a|ÚPowerLawnone?à
!¦˜Ü?ÓãÊèúˆz?ßÉå¼²ÎI?ÓãÊèúˆz?ï	ùɸ£Ô?²ìR¢Çè"?žÀÆÈ녎?²ìR¢Çè"?ã/
ä#o`?½é´Æèÿ€?Ù¡ê7¹!A?½é´Æèÿ€?ïbÿßÒ@³?z}kè'ÅO?" þر´?z}kè'ÅO?о6"*—?ϲQV3é<?ç äîùêµ?ϲQV3é<?æl¬n®?Ë눀'éº?Ó'î§Ï"¤?Ë눀'éº?Üq§@åè?ÁY~%%?áÇ,_õ?ÁY~%%?êp^—Ž²?¶†€‡*Õa?Æ>…£åÅ9?¶†€‡*ÕaMIXED3FGL J0855.4+7142@aÄû~ÿ—@Aœà\̉±À9²õÚPÀ;¾½Žkh.?Ê*êdbU5@_ÝË¢«;@"5`4>¿âÙ±8¿æËÜ2¬‹Ë¿æÆCG¿ïÿêaïD'UNASNone@ˆ
Ÿ¾vÈ´PowerLawnone?ïÿ-Ûc6?+èÀ.qÊÖ?DgÇ÷?+èÀ.qÊÖ?ïՋ8ò~§?ƒ¬R=kn¯?u:cs'ܦ?ƒ¬R=kn¯?ïµ%QPÞ?wï=3íæ?'¶«¥ñ"æ?wï=3íæ?ï·/Ä5Eÿ?c7&v¦?'4ú•š?c7&v¦?ïÿµ|º? _é)Հ?	]h«žn? _é)Հ?î҆ªÔt?®b%pF?¢×•QÜ!Ç?®b%pF?ïÆ©'M3©?€D̔–ñ?|«7i4_K?€D̔–ñ?íºµaæ?¡óûڄÛ?·o")y	Ò?¡óûڄÛAGN3FGL J0856.4+6429@bÔ_Eà´á@BÏ …±…IÀ:wÖ²ÿœ-À;þ¿:=°¿£	ëû·@±¯ØuLˆ@iƒÿÔa¿ê_]Zùö§¿áÎÂ7óaa¿ã=ÞNn;â¿âˀR[þ•UNASNone@ˆ	‹xFÜPowerLawnone?ïÿŠ'á'x?
=¯'?
_9–-Ýa?
=¯'?ïÛ>z±n?'ô+*|?r}`à3ì ?'ô+*|?ïÝpÏS˜a?e3}kr¸,?qG˜>&‹˜?e3}kr¸,?ïëBfµtI?Iøž©¥2°?d½™(/žÿ?Iøž©¥2°?ïþqڅ>?3C¢O7É}?(âY/.j?3C¢O7É}?îö'"dÓ?®"Ê.»=ÿ? –ÖÁyNÏ?®"Ê.»=ÿ?ï}ë6U·?"³DªBÎ?B™8½å?"³DªBÎ?îñDÑÉ¿Z?'ÓÂX ? ë²ãd
c?'ÓÂX AGN3FGL J0858.0-4834@pÊÅXd¿þc@A8¯À8÷0t<ÿÀ:T¹¼NÐH?ðjÓ*‰ìR@
âjé,)@•ô@")›¿é¬p®i¿Þå;j܏/¿ízíBIb¿æ#}"ÔÕIUNASNone@Ÿyç†Â&PowerLawnone?Î@±i!µ:?ÕiªŒ
Ès?èoÓ¥·'±?ÕiªŒ
Ès?êÚŸ?1?ÅúP¾‰h?Çܗ¡ƒ;?ÅúP¾‰h?ãm™ÐÃsÕ?½Ñ߹±?Ù$Ì^yV?½Ñ߹±?êz½ýš?£rÀĄ=?Æù‰˜?£rÀĄ=?¸•1Æɲ?Å~èj"z›?ìíYÇi?Å~èj"z›?Ä­!¶´­?Å \kæ­ô?êÔ·'RþU?Å \kæ­ô?ÚôúÚ7¯?¾è":_?⅂'ä@(?¾è":_?ÒhHœY›?º^X?æðKÛ±Ó2?º^XMIXED3FGL J0859.3-4732@pÀ
»Då¿ð¸±§­X"À8±öFBÚpÀ:J­wœï?ëñ&D§Ã@
2L["e†@^¡`^x?š¢öÛ+C׿ërò·~B6¿ârKuãö¤¿êM|œÖUNASNone@Ÿ"Þ¸Që…PowerLawnone?Á´M‰?È}"ÿ{˨?ë ì¹»?È}"ÿ{˨?êY±Í?ÄóPwÅ<?DZú™8ˤ?ÄóPwÅ<?ââÌà»9?·³Aɬs?ÛÐ:f>‰?·³Aɬs?êçù¨;âž?›Î ˆ+u3?Ä`_uˆ?›Î ˆ+u3?ÃÕ.×?(?ÇX±$®=É?ë9
´J06?ÇX±$®=É?Ë&ß³x?Äí²]éH?é6H?!ÿ?Äí²]éH?ÙQ¹kF?¸ÛíChI:?ãW#J\ðq?¸ÛíChI:?ٞ÷Å|?±¹§ÂVp?ã0ð"AÀ?±¹§ÂVpMIXED3FGL J0900.0+6754@bL"‰a=@Buk¹Œ~(À:ùÂÏ	À<´æüù»?Чɧ‡@©(ÃBµ\@è¶à|W¿Û|õĒÁŽ¿ä7æN†©[¿ÜÉnûØ b¿ïÿ™äOUNASNone@"£2þÅm]PowerLawnone?ïô‰v$¹7?T½¥Q-¦?VíèòX?T½¥Q-¦?ïʊÔɊ<?…2/€ŠÏ³?zº•ÍÆ*?…2/€ŠÏ³?î›4œÈUÍ?"µ%9–Ý?¦L¶2ž¼-?"µ%9–Ý?ïXÏaI?vÜ°™2:?"æÜû?vÜ°™2:?ïÍ?Í0±	?'…>FûO·?y`d7߁?'…>FûO·?î8ƒK›×?µ	Áص¶?¯¬wεވ?µ	Áص¶?ì¤=¤Ì·?¬ºëøÜ×#?ºÞßšJ?¬ºëøÜ×#?êH[ÍÊè`?³¬Õݕèw?ÆސÈÔ^€?³¬ÕݕèwAGN3FGL J0901.0-6725@q·}'ÔÀ+ˆ}€^_1À:D!BoçÀ;ºÉ«¿ñ0Ìxéö©@
AK<>u@0ـ9vC¿æS÷'.|{¿åƒéY€ú¿è-h+•¿äGïç?PUNASNone@ˆüç ù	lPowerLawnone?ïúèðޓ¸?ZçõÉ "þ?D\<vÙ4¯?ZçõÉ "þ?ïÃà೒?èõ¾wc?~³Ev?èõ¾wc?ï "øÛüô?€OQž?‡÷AÌp^÷?€OQž?ïþ‡Û^¾…?¸©@;ÈK?''JDx—'?¸©@;ÈK?ïêX>cµ?m[öƒ¦ÿ?e§ÁÇÿ?m[öƒ¦ÿ?îgÏLƒç+?¶]¤ôÄ/?©ƒ:UBP?¶]¤ôÄ/?îÓ±Šüó±?—jOš–"?¢ÄçOTÝð?—jOš–"?ïÕìk΅?qEûPZ˜Í?uv‰¿Éét?qEûPZ˜ÍAGN3FGL J0903.0-4826@pÑXDЩ¿òÛç‡c60À8ÓÝËø'wÀ:Y8Ëùh6?õ(Ve½I!@
3´k×êb@¼2@·?ê?sÃq.k¿êIˆÆÒP´¿èLd¤LD¿ïÿæ
æÀUNASNone@– !–R½PowerLawnone?ÁÆuZJ#e?ÄÖĐpِ?ëŽb©mw'?ÄÖĐpِ?»
ØÝ7?ÂïlgäÃ?윤äY?ÂïlgäÃ?ØntF»•?´ƒ
V³$Œ?ãÈÅÿÜ¢5?´ƒ
V³$Œ?Õ؅Ô3?°ª?œ1«G?å½u}ç?°ª?œ1«G?«Þ¦"‡»U?ºPU‹€Yà?îB—Ó+?ºPU‹€Yà?–Ê"óð'E?®1à'Ú?ïI«Ø`~Æ?®1à'Ú?ÐB‰žú=?¹á]æU®?çÞ»v°'â?¹á]æU®?®Šýï`sÔ?—‰‡,ùk
?îP!34?—‰‡,ùk
PSR3FGL J0903.2-4744@pÉAÝ!ê¿åߑ€EŠ¤À8­XIm1\À:\ƒ‹:[F?óšzí±ô¯@Å·n–¶@Aäpb¿ìˆÎñÅ+?Ð$fJÑyI¿éKÉ®¤Ÿ¿ç;ý8>N´UNASNone@¥÷†?PowerLawnone?îH^¯ýwÿ?¯"S(Ÿp?«zü¸ä?¯"S(Ÿp?ë!Žø'?Ãi_%e¦?ÃyÉǬø?Ãi_%e¦?çñD&†¸¨?´×#¦˜ó'?Ðw²òŽ±?´×#¦˜ó'?ëŒ|Ћ?¡*Ž?Ü*?ÃùÎ½Ó‹?¡*Ž?Ü*?à—mX{?Ïós±
å­?ÞÑ%ËÛO
?Ïós±
å­?Ô<UM[ÊÎ?ÉÎ""¹ìÜ?åáÕYR™?ÉÎ""¹ìÜ?â3'Öˑ?ºµ6'aÞ?ۘÚSÀhÞ?ºµ6'aÞ?ÜÄ÷Pa ?ºfµ§ÓTb?áó"WÏ0?ºfµ§ÓTbMIXED3FGL J0905.8-2127@o'>E@0òædM‡rÀ9›†g­ÓÀ;}´{/P?ó6Qbô@xè±Ú®@G—¸òпàÍ,×Wû¿ê~²Ó¿éù{ßýߝ¿ïÿJX=ÙªUNASNone@}Ô=Ùb·PowerLawnone?í` yr1Ì?½"n8NÚ?´þü3'Š¤?½"n8NÚ?ÒTO'Òi´?ÉQ^•?Jv?æÕØ7Ë&?ÉQ^•?Jv?ëÊ!³ëï?§(ëÉ)d?À×{Á0PD?§(ëÉ)d?Ý,\ ߕõ?§¢_e1?áiÑï5?§¢_e1?è#†lì?É;Oí?ÏûqæLOº?É;Oí?²¶1[Àæ¨?¿5pi
y?í©9ÔPék?¿5pi
y?ã¯}Óâ¸?ºsÔ›èv?Ø¡X:Ú?ºsÔ›èv?¬—õe…?Ž¼ÈÌ Ð;?î6Ž`Å+ˆ?Ž¼ÈÌ Ð;MIXED3FGL J0918.2-4859@pó¿3‡?҉O_
ׄÀ9.‡¶BFÌÀ:¥£Ho?å¿ÖQ¶@
ÀÍ^m»@†Î¿Á œ¿Ù Ö²÷¿æÒáìĎæ¿ç¶hK2¿èýI¯vz±UNASNone@"Š	ÞPowerLawnone?ë¼Z×<~?ÃãŒÿ¯M?Á"£º?ÃãŒÿ¯M?î5óB
<?¸÷·
‰/³?¬ ËݦžA?¸÷·
‰/³?ëifS¤ ?°{Û®í?ÃÞZf±m~?°{Û®í?í歞‰B‰?‰¦iÄfb?°Ê"ÿÆ3?‰¦iÄfb?ßšâDc?ÒdQç¡?àv²ŽÝþÎ?ÒdQç¡?ÝÙÜv'?ΙÂšÂ?áwy'Äí?ΙÂšÂ?áé*rç¡?ÀUY—Ô{?ÝÒ-«0¿?ÀUY—Ô{?áêõc¼4q?³_H)@ir?Ü*8‡—?³_H)@irMIXED3FGL J0919.4+6604@bvwFˆ{@C¬ü'œýÒÀ:§¢m}±ÝÀ<»%}¿ËDzfoÈ@Øi2ɀè@DÀ
¡©¿ÞºÎ}Q¿×:´Z¿Þï`qH±¿ê÷Ø'D,UNASNone@žØⶮ}VPowerLawnone?ïÒëU+´?vïC¿ÿQ2?vŠUsð¶?vïC¿ÿQ2?ïÜ>ž¡ì?'Õu檥 ?qà°íÂ&?'Õu檥 ?î)â7Ô>?›é"|?§íaÝ^£ ?›é"|?ïëïá"P?KŽ
MuV\?dè^¨
?KŽ
MuV\?ï3ûÙ¶?Žn´€µ#?Œ35êZ˜?Žn´€µ#?ï
ç6…x$?¬'ß»?žC4xei?¬'ß»?í-ÍŽ†U?¨›ä|µÀé?¶''Ð[ÿY?¨›ä|µÀé?ïE3)¼×?ÂQˆXµ–?—Yœ€3)?ÂQˆXµ–AGN3FGL J0919.5-2200@ol¯öÓ0"@3áÞ¬É!À:qÀY÷ÃÀ;¾UË
¯ì¿Ô9Þpì¯Ê@ÿä8¼µ@"ÔÒXR¿ïûM˜†–?ïMÁ`KÞ꿬ŒáõÆ6¿ïÿÚeÌUNASNone@ ¿¼ÓZ†PowerLawnone?îdóʒ‹?¼,Ï'+NI?®‰°Å¥P?¼,Ï'+NI?ïÅ&È
AÔ?‰'# 
Ð?}lœ=
»?‰'# 
Ð?ê¦ÖòFë?®úÐÁ4?Åd¤7ŠäS?®úÐÁ4?ïÍƵ!#?k§‹­YÊ?y¥¢zƒ?k§‹­YÊ?ïƒ3jj?©<\9­Cò?ŸO™@vÔ?©<\9­Cò?î¸}jô7?±ñCwŸ[?¤x/˜î'?±ñCwŸ[?ç–ú$k;°?Àn£ƒŸ© ?ÐÒ·)ˆ¡?Àn£ƒŸ© ?C€ïe?©8$^¯?§';Ã¥†¸?©8$^¯AGN3FGL J0921.6+2339@iœ´¢3œ@Ej˜þi'À9ØüvÀ;°jš¸¿ãðrô
Ë­@FŠ{ïd§?ÿ¢Z± I¿ÐÔò׿´¿áéÈ]ÒC.¿Ø¨b†¿ä<+{.œUNASNone@¢36Ov`PowerLawnone?ïÿó>óÓ?2@Î('…?Á›Á'~R?2@Î('…?ïÞr-2×Ý?'&7ûƒ"?pÆéHWw?'&7ûƒ"?ïèm_[°?eúþïúÆP?g'€¼!/°?eúþïúÆP?ïþ-6¼L?6#è½r?-,'¸7Fù?6#è½r?ïþÝÓ§ª?.÷¢KÎ(?.2ÓAÝ?.÷¢KÎ(?ïBdTß?ªlR®ê?—³u~Ur-?ªlR®ê?ïÙ÷EÚç?xšÃÅs?s{ôoäw?xšÃÅs?ïìm-«?[`W:oÙª?cp௯ú?[`W:oÙªAGN3FGL J0923.8-5154@q=ÈK¿òS;C£À8Íg<O;§À:ÊPrß?â ¸tu7@
GWŎ¿÷@`t	¿ã³íÅ벿ëuÖ?!¿äºáÊ#¾æ¿èÌPi`'UNASNone@Ök@öjUPowerLawnone	?ïpݗJ_?Ÿ÷¨eàŒ?'ýR>?Ÿ÷¨eàŒ?í0–dŸ¬?¼‹"döq-?´{MHö#?¼‹"döq-?íƒoƒ?¢)mÿæ?±ëä'/¡'?¢)mÿæ?í(1t8®j?'ySËP˜@?¶¾t``N0?'ySËP˜@?étEC£eB?Æ:LÐh?Ê.êñrjù?Æ:LÐh?Ö9Âm¥l?ͳƒ‰¦¡.?äã>É-J?ͳƒ‰¦¡.?çj(6ø1!?¶ÓŒh/sž?Ñ+¯'¾?¶ÓŒh/sž?Ü¿.'ÿ:w?±îID?á h¶€bÄ?±îIDMIXED3FGL J0928.3-5255@q1MjO¿ötڂ—õUÀ:_UÐìíÀ;<ÔL?ßcOüÒ@¼HKôL?úgΠ·p¿Ð¶*
ðƒ‹¿ïÿ÷Dx2Ÿ?ïþñå,Œr¿½s54rÖëUNASNone@̖VPowerLawnone?ïþOÅÔÏ¿?.)li‡áÚ?+ .³³ñ?.)li‡áÚ?ïyªb{?¦ÂiÐïâ?Ê¼qøÐ=?¦ÂiÐïâ?ïʺ÷…?| HRA*?zž¢í&EÑ?| HRA*?ïþ6!W>?'B<[qèÈ?,Ÿ›õ+Ž†?'B<[qèÈ?ïùÚJþoÌ?LaÆ°pN?H–Ó\`îR?LaÆ°pN?ì&ŒI2ú?Æ6óö̃?¾ËŸe¶h1?Æ6óö̃?ïžÞ  ù#?‡Ì¬'O‹?ˆHwèïÃ?‡Ì¬'O‹?ïþi×#Ð?3Œë!£?)b¬ÃÐ&?3Œë!£AGN3FGL J0930.7+5133@d·—xW)³@F®$‰LD|À:ÊA{ËRyÀ<!¡t­¿ç'"'åw>@îÔ&2n½@‹ù€_
ý¿è‡>—Y<K¿Ô/¼«Âf¿ÝJ@(l¹D¿äÑäª0UNASNone@¤œÖ_Ø­¬PowerLawnone?ïþ"]€—H?1ò—|ÄGA?-Ú&wê9Á?1ò—|ÄGA?ïß¼Ät—4?'¹«ø3àZ?p!æ°¥±?'¹«ø3àZ?ïÛ*r܅?lEK"^?rjó-ԍ'?lEK"^?ïúœªVfz?4Bd¥÷¨?EWZ+?'?4Bd¥÷¨?ïós¥Ç­Ý?[
ƒeÌ?Y´ñՖ?[
ƒeÌ?ï7/=Ü?ªˆ¦õP8M?™ú"®?ªˆ¦õP8M?︞…^?bÙn?û˜U¹}_?bÙn?ï'‡.e¢?…<´©Nõ?‹zž7Ö3'?…<´©NõAGN3FGL J0931.8+6739@b%M:'£@CâöÕ®À:ZxyŽaWÀ<:§›ºÜ?´>xt鈆@F[oèEN@T1ÿ¬s?¹hBý‰5Ò¿æ	8Ö`Il¿Þ¥LàÙI2¿á7vjP¼íUNASNone@›Òñ©ûçPowerLawnone?ïÿdÕuE…?t§ü¥|?eMo1½w?t§ü¥|?ïÚ^Ü/?ƒM˜þØÒX?rÐüìT‡?ƒM˜þØÒX?ïàŠ;؞<?pn,¼u3'?ouÄæ#õ?pn,¼u3'?ïáá?†¹Ô?R%øX‡þ¬?nÀXIëû?R%øX‡þ¬?ïþô!`‰?!¹½ç÷ ? ¾±ŽZ6?!¹½ç÷ ?îò¾Š®‰?®Â^tCc? ÔUoÄ?®Â^tCc?ïÆGãwá?Ø›cÓvü?|ÜL¶Ÿ^?Ø›cÓvü?îЂxYœÃ?"Fê¹á|v?¢÷Øx®eÏ?"Fê¹á|vAGN3FGL J0935.1-1736@oOö©?)@8²~
ÇÚÀ:#×>?Ö°À;MPëªÞ?ؾ`Èíš"@bŽëjÈ?ûúp™?ïô¡›¬Õr¿åU›d䠿΅.jC<¿Ý
Wna\UNASNone@µ/K…¸RPowerLawnone?ïþ–+ƒš?)—)ì:?&J¢¥íY?)—)ì:?ïƽánç·?‡-™*éÝ?|¡[Éô?‡-™*éÝ?ïÓoFgv?t%®¾V€Ø?vH\Õ3ô²?t%®¾V€Ø?ï¯èk‰?i/؈g*?"þœP¡º?i/؈g*?ïüX—,>?CKæüš?=;G¡Ð¯æ?CKæüš?î}S¸Êó?²T—×Ôf?¨'êÄsPÉ?²T—×Ôf?ï­¯wd)?…€F3?""9¥–'¢?…€F3?îCjÅh!?™PjWŠ÷?«Ï©Qñ¯ó?™PjWŠ÷AGN3FGL J0935.2+0903@lšmÚÏ@D.÷<ÉÀ9àyçLªÓÀ;ÈÓÄ7ÒÕ?õRl>A¯"@׎5bbv@8	cr–¿À.(Q­Ç¤¿å®Wa™U°¿ë™ISþQ¿ïÿÆç'
'UNASNone@ˆFöM½ùPowerLawnone?íÕÏ´fW?¸±xÑÚ?±Wƒ8´E?¸±xÑÚ?ãtå‰uùÆ?Æõ_Q¬#?Ù4ít?Æõ_Q¬#?êϟâ!âm?«ŠNa²®†?ÄÁ€wxvM?«ŠNa²®†?ãLrß
?¦åyï?ÙgãÌAë?¦åyï?ç_Þ¦$R¬?Ì齫>)(?Ñ@B³·Z¨?Ì齫>)(?Ì—*9ˏ?Ç9
Éî²?èÿ5q?Ç9
Éî²?áΡó4?ºÆH¤3¦?Üb¼×ç?ºÆH¤3¦?¿ª.?œ
=Û'ºv?ì|žJº?œ
=Û'ºvMIXED3FGL J0936.3-2114@o³ÿX:S¹@6n¾‰¬½À:`'b"sÀ;¹ö¥ä*·¿ð5§=h@ǽµ'®F?ý|@€M?Àømºm¥¿à
¶¡è´¿×¿Y±¿Ü¾¬3á?UNASNone@°YF$Ý/PowerLawnone?ïþé"_íô?!ËÿE†ÇN?!g½'¹?!ËÿE†ÇN?ïØÖñ=ðQ?'¿‰v@Ž
?s"‡[ˆwÂ?'¿‰v@Ž
?ïß"J'°?p:7µÄ6?pqîõ‹›Ì?p:7µÄ6?ïÿ±·:ó>ôýäŽP»ó?»Ûuó†>ôýäŽP»ó?ïý•J20Ý?3¸ó¡üûp?3U¯5|,?3¸ó¡üûp?ï%«˜¢?¯
½ùbfƒ?›JùŁ¿?¯
½ùbfƒ?ï̘µv¢|?}Jú{æé?y³¥,¡}ü?}Jú{æé?ïüo…Û?8'C:m?<ƒÐÅìv°?8'C:mAGN3FGL J0937.1-4544c@pô ě¥ã@^']Šõ'À9±aB:73À;A€t.¦¿Í.'¹5@dÆ(Bê@닠\¬S¿í°½wš@¿àMà
õ¯ù¿ßÛ[ž"Þ§¿ÞÛÎJv=UNASNone@‹ã4ÂPowerLawnone(?ïþ[3=«B?'c+S"~?*LËk3?'c+S"~?ï²X4ýì2?š‹uÙ9Ü?ƒiòÃD£t?š‹uÙ9Ü?ïÅDD¿?y¨ðšùh?}]ýãÐ\j?y¨ðšùh?ïú×½tGÙ?,_VÌÆ?D¡
‰	Žu?,_VÌÆ?ïøo´)# ?UE3Aʃ?NA/vc¢s?UE3Aʃ?î("6??¹·GN"Y?¯ýv$(ç?¹·GN"Y?ï!ào¤þ?"]ÕÃøZ?›Ãþxê˜'?"]ÕÃøZ?ïΓ95ß>?i¶wÀgÎð?x¶cF#å]?i¶wÀgÎðAGN3FGL J0937.8-6407@qºwÄ\»ÃÀ!"Ê`"À9Ó9¾hÀ;…jŸ±
Ï?Ȑ}l£}"@m¼}cÃ@\Bjy¿âRD###¿ëI"×ã¬7¿ã]W</ŽÂ¿Ú^žRÞ@µUNASNone@†uýAt>–PowerLawnone?ïþ
µÜV"??HEîóWI?/$¢Ï÷??HEîóWI?ï›JeÌ/?—iqÙm6h?‰-fš²¬?—iqÙm6h?ïϕmÔ³?zã;éÛ?x5Iõ?zã;éÛ?ïã¾n˜Â?PýÚ:}+?lA'J`»s?PýÚ:}+?ïû€%̏³?GÚE[wà?Aÿi&Я?GÚE[wà?ì‰Á Šþ»?ÀW`±hÔ?»±öû¨
(?ÀW`±hÔ?®=?Š?ØJÏÛ?_Tt,"â?Š?ØJÏÛ?îÆf"'&f?'DvCׅ?£™–´IäŸ?'DvCׅAGN3FGL J0937.9-1435@o8ÅCk@;48L`À:Kç]qËÀ;¹¤½º
R?ãC^ÿƒ@j3PåJÈ?þ<¶úS?ïý:"£§¿Ù"´¥Â%¿ÚÁlÇS'"¿è°Iۅ9UNASNone@«"A£n.²PowerLawnone?ï÷ÖQõ"ì?Wû,ðo²t?PS\®Š>?Wû,ðo²t?ﺽç?†¾³q–w$?P¬»–a?†¾³q–w$?ï–g¿5H?Š'l,;,?Šf8?Š'l,;,?ï=»4IÜ?xGW©L$?˜H™|n?xGW©L$?ïè!Òb¸Ý?pzLöäˆ?gÞ-}ª»V?pzLöäˆ?îHFÇõÐ?´cŸµps?«{"Ž£?´cŸµps?ï'[ôé?™L/t9?›v 
ñ?™L/t9?ìCA‰ÉS,?£KcÕ¸9à?½åó±µf¡?£KcÕ¸9àAGN3FGL J0940.6-7609@rCóÿ¬*À1lÙÆ°SÀ9?ÎÞ¨À;tOÞd¤Å?½)7ÿD7@ÚÂ-âf@H_•;ç¿æðýlŽõ¿ÞG¿myç¿é›ã±¿ïÿۄ—÷%UNASNone@‹pÍÓØPowerLawnone?åñ7Ñ0<f?Ð2ÜCÀÒ¡?Ԑ]Ÿ‡3?Ð2ÜCÀÒ¡?ï…ÿ®ÿåÜ?"±©«–Ž{?Ž€5·´ò?"±©«–Ž{?é\'Ö#/'?±1Hª"F£?ʍ¸§sCf?±1Hª"F£?îËÔÑöNÉ?ˆ·nr¢ª|?£B²Þ^x?ˆ·nr¢ª|?Ú9B8V*?Ñ՜Ϯÿ\?âþc^ãÔë?Ñ՜Ϯÿ\?é~[\"wé?ȅoÔVâm?Ê'® \?ȅoÔVâm?á`¨˜'?ÁÊéÛbš?Ý?Ì®ÄÎü?ÁÊéÛbš?â­Ó7u?»¤"?ÛƤY'ç?»¤"MIXED3FGL J0941.0+6151@bïu£KÜ@EŸÝ]=ȸÀ:€º¥'ÜÀ<
±qýs^?Ú9üSUÆ@¾{
L¯@_"ŸèN¿êô
$ù)¿âe U,y¨¿Ö¹âÏÃw9¿è–ËFm€?UNASNone@'¿hr° ÅPowerLawnone?ïöâ#døÂ?"ÊnOÑÀ?R;¹;Ü4?"ÊnOÑÀ?ïÑ{]Ìíb?"pðúœÈ\?wBQZ8?"pðúœÈ\?ï½:U'W?…G?Kó³?€±j•Òê
?…G?Kó³?ï€ÈûR?p(Ë0®‰?Í÷ýϏz?p(Ë0®‰?ïðšÛÃi?eGDÒ2ãe?^ÊI¶<?eGDÒ2ãe?îj»!vÐ?°ö_b#&D?©TMêVÿ?°ö_b#&D?ïHysņ?"éΘÝd¨?–üPчOH?"éΘÝd¨?ì<¢r±"w?©†!p&Ô?¾ìjvìF?©†!p&ÔAGN3FGL J0946.2+5209@d7Ÿ©~@GÁÊB®Ñ9À:/þ|rAfÀ<ãðÖ?ä²]Lƒ³¡@ЩIëñ@á'uƬ¿ç/ϓ ¿ç:`ϒi¿ïðŽºå»þ¿ïó¨d@OUNASNone@{lÝDUPowerLawnone?ïéٝ•§?¤_|"à~.?f&b¬Pã?¤_|"à~.?ï!V"'?š©P¢®?›Õ=»u­?š©P¢®?ïb¡_Z?ƒ#˜@•%?"«ÞôT¸?ƒ#˜@•%?ëÂ¥Žf×ó?›#Æ(¤×?ÀõiÆd 5?›#Æ(¤×?ï÷Ê¿_¼?VÜsܺ6b?Pj€yOˆ½?VÜsܺ6b?åzꯋÉL?Ï8Z©2­–?Õ
* èmg?Ï8Z©2­–?îÿòG@íl?"iôxRñ? ۈA?"iôxRñ?ÍR&ޑo?±W…‡oɲ?è«vH[¹d?±W…‡oɲMIXED3FGL J0948.1-3641@p¬/ƒ{J#@)üõ:uGÀ9N]-؀À;"^‡tÔ?얦/ݛÛ@gĹWúé@Æï¿kn¿ç¥ASÈ¿ê÷˜lÀ?¿åJªn÷¿ïÿ²,(UNASNone@w1ŽóMjPowerLawnone?ï³°N;ø)?"…iû‹?ƒìkڋÖ?"…iû‹?çÔó:'vÅ?ÃîgsñX?ÐV‹±v?ÃîgsñX?îbhúâ¬*?˜ë£~T+Â?©ÙpThòd?˜ë£~T+Â?稫(swØ?¢]ÎX¼Oi?Ю©¯P?¢]ÎX¼Oi?ï$øÆ-~ò?žèšVڌ'?›`ç1¹Ñ?žèšVڌ'?Чâ2ËÀo?Î{jžHCÕ?ç¬æšÉ?Î{jžHCÕ?êšs3Sj?³üî
b?Çݖ32²Z?³üî
b?È#¸½‡p³?¦ì¨ÍS?é÷О#Ó?¦ì¨ÍSMIXED3FGL J0948.8-4243@píƒ<`Ÿ@ û¼ÓZ…ˆÀ9ª¨ëF4˜À;u­Ñ_Å¿Úç'euz«@
;R'rY@ñ…@œ'h¿êeÜVòD¿ã9¾dv™‡¿ß0…_a¼¿ê(,"dËUNASNone@‡^9XbNPowerLawnone?ïÏ*6פä?}þGÝÐÝ?xjä‡	Ù?}þGÝÐÝ?ï³Ù*'?5‰*´Õ!?ƒ	µ~±Á?5‰*´Õ!?ï&érí)Ü?² (Ì)?›"ѧ'.|?² (Ì)?ïé£=˜x?Q¨þ2®?f\Â0Ž(§?Q¨þ2®?îéºþ2_?¤>Vãøžž?¡dP N¶?¤>Vãøžž?íñ»r÷M?¸j`ìJ?°r$f÷œ?¸j`ìJ?ìÝÁªëâ£?¦D|§]Œ?¹ò¨ êé?¦D|§]Œ?î´ãoüg?•ÅUñÿ*?¤¾ÇHkŽ?•ÅUñÿ*AGN3FGL J0950.4+7550@`í(Œç°@BD–Ý&·$À:Ö`"•À<=%ÑJàÏ¿ì1Éc‹À"@
óp˜nv@'Í@¿èòW‡´¿ã¡ãÙ?8¿Û™;‡·ç/¿ã¬¬
VèfUNASNone@™¿¥F
¦LPowerLawnone?ïï™"{U?vTa‡U\?`fݙHœï?vTa‡U\?ïߞëµg£?'MÚÆåù?p0Š;I®}?'MÚÆåù?îñV0Œ?ßÒ¬î\«? î:œ
[@?ßÒ¬î\«?ïþÄ\¡ý§?n¡. áò?#º2ȍ5?n¡. áò?ïåtìf;?t÷͚'¾å?j‹tÉüô?t÷͚'¾å?ï5k¦R?«]o>†‹?™\ß·²Ÿª?«]o>†‹?îcPWÜ?¥ºIí}Õ?©Êÿº'>Ö?¥ºIí}Õ?ïêÓ'Úºv?a¡ ?FW?e,ØFÉÜ?a¡ ?FWAGN3FGL J0952.8+0711@l·`—Ì@E¢}sÉÀ:sÐIYÀ;µ™9øI?Ô£xM¢'æ@
jT»ï?û0©ôg?ïùcñÁùµ¿ ['îËi¿×®k@sk¿Û~ˆ&ÌëUNASNone@·;dZ¬PowerLawnone?ïþ_Ôpv?5?·gk7F?*½•¢ÿ±?5?·gk7F?ïÕ	†³Û1?ƒÐÌWzCø?u{<ÁG?ƒÐÌWzCø?ïØi`õ@è?n¹Š3¢Õ:?sËOr!¼.?n¹Š3¢Õ:?ïÏ~Ȳá¿?^¬î®"?x@›·½,W?^¬î®"?ïüSeá8ó?=lsa¹?=dѪŠL¢?=lsa¹?îýÙ(išg?­æ}+‡"Ë? "m{'Š?­æ}+‡"Ë?ïÂñ·ñQ?€=L*ì¸ß?~‡#ïú‹?€=L*ì¸ß?îèl!ޙu?'eÀÁT2W?¡y=߂³®?'eÀÁT2WAGN3FGL J1002.0-2837@pyæ{_ï@5¸Ç\J"À:*ˆ«€À;µØÿàöO?çÇ(¾Žñ@GP×3@œ	ßý¬?ÇVùÌ_>ª¿è`ë'UÚR¿é!ÉÔIï¿ïÿB¸·AUNASNone@'»è]·k<PowerLawnone?ïØ»a%Åó?wÔؼÈ5?s¢OQ &i?wÔؼÈ5?ççB2Ä<?Æ2Oт×?ÑÜ1{šw‡?Æ2Oт×?í-µ…]w?¢žûß-#Y?¶'SÒ?¢žûß-#Y?æ?ë>
=?¦ãsYùL†?Ӏ)ƒå…ß?¦ãsYùL†?ﮆúkҝ?Ý®Ú9!?"^Auán?Ý®Ú9!?αIÑ&Æ
?˯"…G@ö?èS­‹¶N~?˯"…G@ö?ìºÅ 0!0?§¥#Ÿô$ö?º)Öþ~ö€?§¥#Ÿô$ö?¿¤žÎjdU? ¬`–yÆÄ?ìl&2³u? ¬`–yÆÄMIXED3FGL J1003.7-5215@qlKƧïž@–ÎãþAºÀ9Æ)É'%ßÀ;7]ig¢§?íb¹æ±6@˦‡Ù@{>ŸÍæ'¿"±h~Èô¿Üþ?FοåµjlÒ³Ž¿ì•h.èuËUNASNone@•©-w1ÅPowerLawnone?ß®¹™ò¸?ËÌ1=Üü½?à~¨£3¤?ËÌ1=Üü½?íŸj¨â¯/?··
3Iw{?³ª¶ÄÅ?··
3Iw{?ç¸àa˜æ?°ãb(ë»ã?Џà?<Î4?°ãb(ë»ã?íØۊ ?+Œ63â"?·Ù9!‰½"?+Œ63â"?Ç`Œm§è?ÂV«ä±O?ê'Üÿä–?ÂV«ä±O?ÞÉ
byâ?Ë
Ö·v?à›y~NÃ?Ë
Ö·v?ÜË£'ì¦?½À=àÇg?áš.6õ	­?½À=àÇg?âšùÀ÷?°~…P%K-?ÛýòÊ~?°~…P%K-MIXED3FGL J1008.6-5706@q£*\|Ù¿î3†_€>À8&Ô©À:(ÇÅüÎó?ÛbÕh¸âE@
Ÿµâûba@ˆ€—•¿äúEoº'Ñ¿æy™¨s¥¿ëAÀáÿ¿áŒs%¡UNASNone@'¶`ªdÃPowerLawnone?Þ/eÛs{?ÔLu(öï5?àèMFBs?ÔLu(öï5?îæÜ×B,Ü?²»D™?¡'2(µ4?²»D™?á4‰¯
@¨?¼èÊ] ˆæ?ݖì¡å~±?¼èÊ] ˆæ?îí}~RbÆ?†bï¦{X?¡((mˆ ?†bï¦{X?ÄЩj
ú?Ìm35ÙÎ?êÿ‹Õ¥}A?Ìm35ÙÎ?ã'é"Ç?Íøp¡u'—?ÙÌÚ,öqü?Íøp¡u'—?ÚÒhàû>?Á·5¿]+?â–üˏ'a?Á·5¿]+?ä`Î	kl=?½Ae¿¼1ä?×>cí)'…?½Ae¿¼1äMIXED3FGL J1010.8-7645c@r`ï~=ÁÀ0¼øµˆãiÀ:¾7ޓŸÀ;o	µ‹g¨À7º¬cˬ@õ&Ûa:@sð?m©&¿ç–î÷ø}¿ê¬kÉ°@X¿åÖÆ]xÐ?¨ž€Íߋ/UNASNone@š¹Ž_oÒPowerLawnone ?ïúÛ7 f?Jõß-Å\?D"$›9i?Jõß-Å\?ïÈ®öUºÐ?g,æ¼,Ú?{¨"ìïË?g,æ¼,Ú?Zx¿?~Q¡üFf?‡]<úÜ4?~Q¡üFf?ïÿÿ€Â÷Ñ>"'Š-Uƒ>Òã›ËÁ	>"'Š-Uƒ?ïßDU^ã?uûÃ	†?p]Õ\4&­?uûÃ	†?î¯9ÚÓ[î?³ÎNò SÅ?¥bP6Œ?³ÎNò SÅ?¹SY€?žM'ÎÜîï?§×"jÊh?žM'ÎÜîï?ïÿè—û×>ò¨¸±]ð~>çg¹š™Z>ò¨¸±]ð~AGN3FGL J1013.4-4008@qRÇ%Ä@*µÿÅGÀ:=©µpµÀ;ª\™'6¿àvÃá@3%>Röó@Æ ‹:Ü¿ãM-M:¿èw/òêv_¿Úzƒ9L¿Üщêc®UNASNone@™´äZ¬PowerLawnone?ï­¶³Ÿ˜ü?¹YV€L?"'S)GÌó?¹YV€L?ïÌ[m—'?ˆé–G"ÂÖ?yðRaA{…?ˆé–G"ÂÖ?ïËÖ°6¥?ƒŠšV˜<?z~"Ê@Å1?ƒŠšV˜<?ïýߣWø(?Ýöÿœöû?1æ¨â‡à?Ýöÿœöû?ïþ7ž&ò?.-hѳ̒?,†©ùÍ?.-hѳ̒?îëœ7Gƒ¼?²,'R]Îp?¡F<Ž÷`<?²,'R]Îp?ïy¤oœ¬/?'§|íL°C?Ër'ä?'§|íL°C?ïç«'<?`¢C V?hôU ɜ<?`¢C VAGN3FGL J1016.6-4244@q/È÷Q@'%WšñˆnÀ:#ÜHjÒÝÀ;'Uœê†ò?á;Ó*½@x|¦CÌ?üƒÒÀVǸ?ï±jØÞJp¿ãæh4æe¿Æáâ	í6¿Ú0âÿ$tUNASNone@´'{çl‹DPowerLawnone?ïþÉéºæ"? ¦¢Bú?#abtf°P? ¦¢Bú?ï¥aZQÉæ?žY`"KnA?†§©uÜZq?žY`"KnA?ïÛGxSg ?sÝIž»â?r\CÛ¤?sÝIž»â?ïâI4J?R¾A|¹U?mù¶Õ‰Å?R¾A|¹U?ïþoݑÓ?(4€ìg‹?))…~?(4€ìg‹?î!:ygcÖ?¼ÚÑ9´?­ìXi‰Â?¼ÚÑ9´?ïÏ:‡)C_?|œÓ'ŠT?xb¼Tø–?|œÓ'ŠT?ïq5Þos?uëW	¥½ä?ˆ£²–"">?uëW	¥½äAGN3FGL J1016.9-2653@p"æ1ø @8sÀµgUÀ:ùã†MÀ;ÁSL®.|?äøã#%t@F,6ê¢Ì@×(Ÿ[zz¿äšèù=f¿æ
Hy&Ä¿ê²!óR¿ïÿå|WO®UNASNone@z^5?}PowerLawnone?ïõ•³°ñû?^ÓÓcÙ0?TԘk[?^ÓÓcÙ0?îLu¦5è?¦íх<l!?«8¥Ÿ¡ˆ?¦íх<l!?ï)RgM?Š2ÓÍ·?šßÿ—jäQ?Š2ÓÍ·?ëJˆØ^ÙÞ?™>ÿñǕò?ÂÕܞ"˜‰?™>ÿñǕò?ï×#C?.u˜
]ß?tÀW_?.u˜
]ß?àÇ€I]ä?ÑVGô¥É?ÞqðÿmD7?ÑVGô¥É?íû>§tg?¡¸îT¤™?°'Æ2PD?¡¸îT¤™?Ïýê*o"?¬'Ô›‡·B?è…udý?¬'Ô›‡·BMIXED3FGL J1018.2-6254@qç"ßÎ1QÀ'C¦GýÆÀ9–©$Q!À;A#·;k?='9@)ÿæ)À@Š½¿¾œ]¿çXQ¹—L¿ì¯ \†ä¿Üi"Ei8¿èø²JYYQUNASNone@‡ö§»/ìWPowerLawnone?ï}ÀMÚÌ?¡W³‡kŠ?]gûl'?¡W³‡kŠ?ã͑0!?͍/,W:¾?ØdÝçɟ¾?͍/,W:¾?îɕ(å"?–i"ò"¥?£f­y™u½?–i"ò"¥?é­Ô›?¤ö8	Ä?ËíH¯é‰"?¤ö8	Ä?î²-—<òû?¬3O'‡ç?¤Ý&Œ0ÐW?¬3O'‡ç?¶Šçä8í?¿gìr–?í.£OÀ³?¿gìr–?ë,­¥?°MTIªÚ9?çMI½kä?°MTIªÚ9?ÒÓoä>ƒs?·˜4d—¡u?æ–H
à¾F?·˜4d—¡uMIXED3FGL J1021.9-5815c@qÄó#x«
¿ìùcÞ÷œ¯À8‡7ø"Ñ´À9øîº]^€?ò¬g|õ@
pò\ÔA`@iŸè=A¿ê¨ßp¤"¿èPÒüøʾ¿æ?˜°ªF)¿åX£7ÜUNASNone@¯ôœ"µÜÆPowerLawnone1?¾ë"Y"}?Å)Cõš™?ì"›¿tÛ°?Å)Cõš™?燘E[ª?Ì7íÍM{3?ÐñôÏuH¬?Ì7íÍM{3?ÛcÀQÇÑn?¶¸`~ ë~?âN×I?¶¸`~ ë~?éø×	f±?£Û½hqR?È£Úe;Ä?£Û½hqR? Ù²¨þP?¬ãÁÌaÄ ?îòdÕ}܋?¬ãÁÌaÄ ?¾!º\T60?®
ï׿?ì;È´uy:?®
ï׿?Øñþ"bÞû?¸Ã;¼_:z?ã‡îΐ'?¸Ã;¼_:z?ԋO?·ê)œ¢Ñ?åºr·Øsõ?·ê)œ¢ÑMIXED3FGL J1024.3-5757@qƌ½D¦¿Þ)VÍÀ9š‹1!
À:.Ü:(ú¿Ñ>ø­jÈ@ò¿[Ëñ?þSé Àiè¿î;[¶4/¿åW#P?Å7ÿÒø0¿â¾ôUNASNone@ɬyº^5?PowerLawnone?秓xÿØ?Ñ"SxfÞ?аÙÀO?Ñ"SxfÞ?ïyoo¦V?¨]£)³?Òk+ýG?¨]£)³?çc*8º©?´iÖˆ¿?Ñ9«éŽŠ®?´iÖˆ¿?ïù¿K[?H¸È!Êu?I'£ÙB?H¸È!Êu?è`‰`͆l?ɶÚáÒ1T?Î}Ú|ÉæO?ɶÚáÒ1T?ì:²ðúöÎ?Å|6ºÚº?¾*hx(I?Å|6ºÚº?êfÛÎU
?±Uړd_?ÆdÇÒ«Î?±Uړd_?ïáϹnÔ¨?k–"·›Ü?n0FWqè»?k–"·›ÜAGN3FGL J1024.4-4545@q]¼ÓZ…ˆ@#®šõº+àÀ:dú:þÀ;­â1¸ß°¿Ù	­Ä°ú@
CËPuä?ÿmVàa!¿änkͥݿèëÀJˆdh¿×ÄöCÏÊ¿s)â4d¢UNASNone@²ÅšÀƒoPowerLawnone?ïÿÿq˜Q?"€¥O¯ê?€©›'¾?"€¥O¯ê?ï½ó#l?s`Äè?€ƒ:éÕ+?s`Äè?ï✾V?m:ئoIö?mécS‡÷'?m:ئoIö?ïÿ(Á.!ë?
0ü´ÁD?çޘÝ.È?
0ü´ÁD?ïþ
6S"?1™š
LÈý?.OZD¤nI?1™š
LÈý?î›1
,ýÿ?´ÉiY©Í?¦Lï,T9?´ÉiY©Í?ïÕêêçap?zÍ%A=ò?u
ŠŠ?"?zÍ%A=ò?ïöqÙ-¥¢?P)äYAl*?SM+Â|˜?P)äYAl*AGN3FGL J1025.1-6507@r#9ÀëîÀðÞ	52èÀ9g½ò>v]À;OÅ?é$?ð1©J¼'Á@¿r/r^l@Y© ¢ÍJ¿ä48/¶é¿ç
Šån%Å¿ïõ2\¸"?ï!¦mèfUNASNone@Œ†T,<žíPowerLawnone?ïä w?¯€Ø¼öê"?#sÄë#?¯€Ø¼öê"?ïÅý§?ž†Ü÷"?@OÌ'(?ž†Ü÷"?ïK'Š^h?$ž£wF'?œV¬üdú?$ž£wF'?ïø%ב2(?PÉÞ)ÇFÌ?Oh¡úüëÂ?PÉÞ)ÇFÌ?íYîä'\?¼LFŸgÜ?µ0‹ò"»?¼LFŸgÜ?ë1?	¢Ž?ǂw
šÛ?Ãë;ÙuÊ?ǂw
šÛ?ëdp,Ò'?¬cÎ×J†?Ân?Mȵ¼?¬cÎ×J†?ï1&¤«?§¹IÆÊ3¨?™Î.ï& ?§¹IÆÊ3¨AGN3FGL J1025.7-5659c@qÁ;÷'?ÜÓ¢©ã"À9·
èaÀ:O|N/7ü?è
j®–ù#@U¶öv¿O@'Ÿûž¿ã]+Í}¿ë@%§ô¿êöü²e¿äZW'=°UNASNone@§mpå`A‰PowerLawnone0?âî";ǵ?Õ)ØãÓÆÞ?Ú#ñ»ˆp–?Õ)ØãÓÆÞ?þd–Ð?µÑ'ÁS´í?¥÷ðna?µÑ'ÁS´í?ã݅ìŠú'?¿Lx¥>yŸ?ØDô&ê
Ü?¿Lx¥>yŸ?î¶Ëu¬ ý?†íUÛ6Ì?¤"H¦×-?†íUÛ6Ì?Ír¢•Ý*?ÑX
Cp©?è£W{šˆµ?ÑX
Cp©?àÓ
ãw¢é?ÏØké'd?ÞYê9º/?ÏØké'd?Øù̏+\?Ã#[2ð\
?ヸ7êR?Ã#[2ð\
?å‰EäeÆ?¼"潟ïZ?ÕÊít74u?¼"潟ïZMIXED3FGL J1025.9-5930@q֍"M;¿úûh÷:^¡À9õ@‰]À:vc ¹HŒ¿ù\·%Eµ@`?
1@¼¿Àéz¿Û3_Œò0"¿åT]/¹‰­¿í\ºPüпÏeo+ÃUNASNone@¬I"ýó¶FPowerLawnone?îÕÝË*hè?±gI_¹[Ó?¢¢#Q¤ô}?±gI_¹[Ó?ïžÝ[˜à•?—ÕKh·Ž?ˆH©ÇÚÓ?—ÕKh·Ž?êßÚ¤.|?°T'6+¯?ÅȀ•oF?°T'6+¯?ïÿï7õ~Œ>á͘ë©G>àÈKrÕ>á͘ë©G?ç3è3
Q?Èwc¹¸Èß?љà/™å^?Èwc¹¸Èß?í F{(Y)?ÂPEُ9*?¶ýÌ&½6µ?ÂPEُ9*?çwk(Î?µ»Ð¾-~'?Ñ)á®cß?µ»Ð¾-~'?ïýu"e?9vŒS¢?4WżxD?9vŒS¢AGN3FGL J1027.8+8253@_øA [À@@e¡"úÖËÀ:y¤O\_À<çCp˜?Ó»v«Ô/@
ܲ6žw¥@•¦_Р¿ã¼Ê}+¿Ùw£—–¬w¿å臿Û<÷"œô(UNASNone@ ¡ä÷eþPowerLawnone?ïû.;™‰?T‰z'8pŽ?CGÿé¤Ä?T‰z'8pŽ?ïÖ!PîÁ?ƒoÀ£•?töïHjWƒ?ƒoÀ£•?ï»Åìûw?tƈÍ/ÿe?…F4?tƈÍ/ÿe?│šú}ñ?d¾ñRÍ1>?€ÙQ†­ž?d¾ñRÍ1>?ï¸4£1>?"Å"_¨8?ò×@ÈW?"Å"_¨8?îéËFv?±K:.,Á³?§ácOä!†?±K:.,Á³?ï$Œyr?•'rçCÀ?›}gQ m¯?•'rçCÀ?ì‡q/[üð?¬‰r'?»Äv… '?¬‰r'AGN3FGL J1028.3-7419@rXú$‰LDÀ,=Žc|À9ê)€,À;X¸þ¹¯¿Ê›IÁƒÝ4@OFǏ¡@…:Ÿc2)¿ä¬Ú¼N¥U¿éÝ\0F]¡¿âHS‡Ö<|¿ïù۞ÕKTUNASNone@|Ãð:û~'PowerLawnone?ïã}ߐ+?kæ¶I|ò?l' UÞÍa?kæ¶I|ò?ï§6³t ?‰âÖõ%Ï?†2SC±Ì?‰âÖõ%Ï?î·²Ý"?'Q™§eÇö?¤"Ò/‰ÆÃ?'Q™§eÇö?ïŽsùÕw?sìeÌì
?Œc'py?sìeÌì
?ïÍþ°Gº?{ÓzñØÜ?yñ	Ÿ"g?{ÓzñØÜ?ë@ö¥ìÁ½?ò‡B:Ha?Âü%hLù?ò‡B:Ha?î6 ÿ¥£N? ?Ԅ»¶Ü?¬•ð9€? ?Ԅ»¶Ü?鬩AÏÙ?´ó˜2L?ÉM['øÀœ?´ó˜2LAGN3FGL J1030.0-5809@q҂ýuâ¿Ï¶™šróÀ9žü¯égÀ:H?³t63¿å­¯è)cj@Q>kµ±?ü­9~ÑÂ*?ã}M\¢¿æ_µj¿ç«®TÅ1ֿјšbŽ·áUNASNone@ÎÏÎV"PowerLawnone?êûàéßà?Çpâ­×
¶?Ä|[è€?Çpâ­×
¶?ùÞ?¤ãbƒ‹må?ýÙz©@5?¤ãbƒ‹må?ça%švìÏ?·R˜êý?Ñ=´Ë&b?·R˜êý?ïÿoêH³£?æŸêAu¤?³f•®x?æŸêAu¤?çVæÜöï?Ëy2›Þ˜Q?ÑR2F!Ú?Ëy2›Þ˜Q?ìº
±)¿R?ÃæãuÍ?º/'v²n?ÃæãuÍ?è@(Ú>ÐJ?³gH²z1?Îÿ\—¾×?³gH²z1?ïøS?åj ?LSè	_aŸ?N³D	ŒQ?LSè	_aŸAGN3FGL J1031.4-5855@qÛXâe,¿éôّmäÀ9/Q˜y*À:^2»>/?â,ù|rE@
­o‡l@®<_Å½?íc·yBP¿ÖËïΣ'¿ãPÊs^Ïø¿ÚY°~7UNASNone@µݞƒä&PowerLawnone?ï†)1Iž?—~h^åÈÚ?Žu³»wȋ?—~h^åÈÚ?ï]Š¨B²?´a풷t˜?Ÿ4N³Ž¯¨?´a풷t˜?í]GÅÖ'X?¦ÀÛÏ_~_?µÁÑNÅ>?¦ÀÛÏ_~_?ÜÍ??r­Òà.øÀ?ŽS×
DA?r­Òà.øÀ?íe/"d?´ é8Ž?´Ö‡GÈÆ¢?´ é8Ž?éHûk"n?Ê®BFü?ÊÜQ³žJ?Ê®BFü?ë·B>
t?®)ê)å?Á"÷Ö/™?®)ê)å?힣ĕÇ?¤hM,"Å?·
à'wM?¤hM,"ÅAGN3FGL J1033.0-5945@qäîcŠ	¿öÃdٞlgÀ85׈±ÙÀ:k qäI?ᬜg`@
*l!à@	ohی¿Á žXùžð¿çe2´³%‡¿èK4ì=Lß¿ê­ò$'ÛUNASNone@˜Nl‹C•PowerLawnone?áfZǸI?Ð
.MyN?Ý3Jqào?Ð
.MyN?ìh*ä㢅?À£VÔ•?¼¾¨ØâëÙ?À£VÔ•?ãÛÇ5«í?´òèÓ.3ò?ØHq"©%?´òèÓ.3ò?ëquN>Z? jpJæ3?Â:*Ç—Ò? jpJæ3?Â+5½
?ćŠ:"ˆ
?ëu2º¼™?ćŠ:"ˆ
?ÒöÔ5qX?Ëñò˜…¿¿?愕å@GT?Ëñò˜…¿¿?Úx}p?a?ºy!¾i?âÃÁ|GàP?ºy!¾i?ÒIÊÎh?±C}è"ýž?æÛ1˜÷L?±C}è"ýžMIXED3FGL J1033.4-5035@q›—Oß;@	U./¾4À9TãqT2À;_	ðCÊZ¿×QÏO!êû@¹ÿ´€¥­@'À
¼Ç¿ç³ÜæËQ¿ÕP¾Î M¿ÚLfó •ï¿á¸äÒAUNASNone@¤V"µÜÆPowerLawnone?ïún\:NÂ?A]¤š4A)?FFŽã¦¿?A]¤š4A)?ï±½=så?'3 žú	O?ƒ°¢®Åî?'3 žú	O?ïÐp¡}¿?sCÁ&ϘF?wúG•ÔÕ?sCÁ&ϘF?ï÷éìjÖ?:¡ªQÁÚ?P,'íÀ®?:¡ªQÁÚ?ïðy`zOc?W'SY
^±?_
?<ۚq?W'SY
^±?îh³®ÔÐ?¹^I´?¯¹tŲú?¹^I´?ï–*AQ¯?‰(M'èó·?Šu}!í$V?‰(M'èó·?ï£ÖVccþ?yvûo܋¤?‡
jg' ?yvûo܋¤AGN3FGL J1034.0-5731c@qÔ·éùr?âQ+6¯ÆÀ8‰Sԓj«À:m;Ì^èÄ?ñ7œvë¼@3Qƒ«E¾@D¨ƒñ?ïþoïÒ
y¿êBpI³—¿åMÞzýªÄ¿è´MŒÐ³aUNASNone@Ÿ<àA‰7LPowerLawnone0?éòd¤¢ê¯?ÅC²)¢*?È6mmtUE?ÅC²)¢*?ë">A"?ÃåAË?Ãw§û­ò?ÃåAË?èHÑÙ.¸ƒ?²†Êô€Q?Îܸ›Eõ?²†Êô€Q?ë¤oõ—Ç?Ÿx݋Þ?ÁnCà) ã?Ÿx݋Þ?Þê…ÐdK?Ñþ¢>у?àŠ½qÍÛ?Ñþ¢>у?×ӇnSÇ?Èé¸üòj§?ä<HõV?Èé¸üòj§?Þœöà
†?»dÞKy?àý1"ú½?»dÞKy?àÓc)ù>?µ*bPf§?ÞY9¬ýƒ?µ*bPf§MIXED3FGL J1036.4-4348@qjÚãæÄÆ@)9+6½+À:(ÇàÔÁŽÀ;²Y¥Ã£?Éx§À'›'@
‹+ÅUµ@6èßÒãè¿êbägYfµ¿Üõ>.þ‰ø¿Ñ2VG¿ïÿß¡ï1.UNASNone@"'4‡ü¹$PowerLawnone?îù‡yl¹£?¤$yà ·Â? gˆhX~Ó?¤$yà ·Â?ï™4'Ø8?'©"Ó³~š?‰²Û|@ö?'©"Ó³~š?ëê@•òE,?©¯6ÞÀ="?ÀVý¨6ëO?©¯6ÞÀ="?ïFlb¡,W?~¼XTÆ?—2s¦³?~¼XTÆ?íúñê­LC?´bMVñm?°(p©¹¶ë?´bMVñm?ì@"ˆÞ`s?Á'3ΆÚ?½ûc¹üh?Á'3ΆÚ?ç¹Í*¸ä?¾è@Že‰?Ќeªò7?¾è@Že‰?ê`¦{RF?¸sã
Â:—?Æ}f¶ê?¸sã
Â:—AGN3FGL J1038.0-2425@p¿á2µ_@=;qdÇ)öÀ:29Úí!À;ÇÏ'ðßÒ¿ôtÞt"ý@PÓw`ߔ@,\@Gù¿çO•ßR¿ãlnÌ&J¿èøʕÿŸø¿ØFc]˞UNASNone@(ªdÂø8PowerLawnone?ïýZõ«#–?C¬Jòî4?5(R'X7¬?C¬Jòî4?ïÜZÃ^Óº?'­ý,ÿ¦?qҞLv›&?'­ý,ÿ¦?ïÃá¾÷L'?xˆìG?~ qÌt?xˆìG?ïÿáë©!>ã
Oº[¸>î-xÈ,¼>ã
Oº[¸?ïùVeå¤?Pð‹¿£…â?J¦jÿhöë?Pð‹¿£…â?ï@A—¶%Ó?«Òøٝ?—÷Íªáª?«Òøٝ?ï[ÿÓ	|Ö?_à‰nÞm?"€™¨û:?_à‰nÞm?ïü¼$ø¡¬?:ô¤ª¶L?:×û-_?:ô¤ª¶LAGN3FGL J1039.5+7324@`׆`ÔV@DG(àÉÙÓÀ:fK†ýÀ;éäwä=,¿÷æ©IåÒ,@ˆŸã	Ð
@À6 %#ü¿æ6…sO‹Œ¿ØŸ¹ÌÈx³¿á¤ºiÈƃ¿ãÍ
ñŸÿUNASNone@¥Õ–E¡ÊÁPowerLawnone?ïÿ‹XŽ6?à‹þ³6?
)ÑgKÈ$?à‹þ³6?ïàú4u8Í?'6b ÉD?oËmêzÆ?'6b ÉD?ïïˆ9±ä?cý>²Žü?`wƏ‹Ã¬?cý>²Žü?ïÿì"8Ë4>ڊ!F´-ø>ãÝÒ
»À+>ڊ!F´-ø?ïÿR16j?‰­iNÎ`?¹Ò 
ÿ¦?‰­iNÎ`?ïAÎìâ–ä?ª¡ä'›˜?—Æ"^…¹–?ª¡ä'›˜?ïæ[+Ë?s¶­±ï?iôëŽÖµj?s¶­±ï?ïþvðø%@?(ë֎5G?(îÓ²Í?(ë֎5GAGN3FGL J1040.5-5926c@qï™Ã‹«¿å¼^pÐÀ8À,ºs-õÀ:KŒÚw?ì/±>âúó@}Fößoè@U— E/_?ïÿÒ¯Kè¿çœ>˜ÍÔ¿è·ÚÙ8C¿édz"o!UNASNone@±¼ÿ—$tPowerLawnone5?Ü»gÝè[§?֋ÿŒ+‹¹?á¢LÒ,?֋ÿŒ+‹¹?æVw僖½?Ë
òu0ŒB?ÓS4ø҇?Ë
òu0ŒB?áZŽ¤ý?¹ROÜãЇ?ÝKôâ·è?¹ROÜãЇ?èbôAô?©~öÓw?Ît.ûëô/?©~öÓw?Ú¸ø"Õ±½?×
	ߎÅ?⣃î•'"?×
	ߎÅ?Ã%Uð!ž?ÀÿÑÒ>›?ë6ªƒ÷›Ø?ÀÿÑÒ>›?ÕÜ/¤!L?¸™r"µ¡?åþh-ïZ?¸™r"µ¡?ÏmNlʃœ?³†ÓÜ ;?è$¬dÍ_?³†ÓÜ ;MIXED3FGL J1043.6-5930@qõ¢£Y6¿áʇ㎰2À8'oJ:¶µÀ:ɵÁ?ï¬çÁ½¡@˜ü§…ëg@†ü L{¯?ïïð`OËð?Ø{W­C£!¿â¯G›¿àõ°Ý)UNASNone@¿¹öOv`PowerLawnone?àR%`P''?ÐÓyÄ<0?ß[µ?^Üý?ÐÓyÄ<0?è7$,b½?É¥
`eÆX?Ï#oNu£?É¥
`eÆX?äñD(¬z%?µ•r_ÇO…?Öw®§·?µ•r_ÇO…?ê'
ÂqT?§&žZ‹¡:?Å»×Üö:¯?§&žZ‹¡:?Þ0‰×üù?ÍzöÞn5?à练}?ÍzöÞn5?Õ}‹*j?́­ó |*?åAxºj¹K?́­ó |*?æ°¿õŽ?³µšgòC?ҟæÌã?³µšgòC?àV\âÞ<?¿Ú'h¶³í?ßSF:ÄC‰?¿Ú'h¶³íMIXED3FGL J1043.8-5851@qñDЩ*?Ÿ2±zƒKFÀ9qÁ
|À:¶,A§j=¿ãx×Ko®Ó@öôØ·›?þÒ_‡$!¿æÔ)9¬–n?ìS¤øûÝd¿éúvÚ¡X¿Þq'>|UNASNone@ÂQK¥ãSøPowerLawnone?îÀ}:"O?À'2Ÿ0ÿŸ?£þ¸(ç/?À'2Ÿ0ÿŸ?ïy(­À?«VF°)L?Ý:å "?«VF°)L?ìù'¢¦Õå?§6ýÿ0–?¸3jì+Y?§6ýÿ0–?ïù)'bùÓ?A¾eþžA?KY÷'"ŒW?A¾eþžA?ì| Y^8?Âñ";í¨?¿dý5C?Âñ";í¨?ì…2Ü÷o?ĉ}Óъ?»ÖiGt‰?ĉ}Óъ?éÞԒ©‡?²Ð¸4|mì?Ȅ­·'Yã?²Ð¸4|mì?ïyÚÄÝC?mܑ
àÌ?Ä§[Æq¶?mܑ
àÌAGN3FGL J1045.3-6414@rIº^5À–§}‡ëÀ99ÀgmÍÀ;ú¶êã8?ôœÙ!™Ø¯@Ép륀@êvà1-Ÿ?î…а噿è5q—Ù[¿é°9é'BÜ¿í ¯"VU;UNASNone@Ž½¼ÓZ…ˆPowerLawnone?Ðjm$›–?ÆeªÖÐ(C?çÊõIm²5?ÆeªÖÐ(C?É4æ«_´?Æö!''?é²ÆU(?S?Æö!''?ã[H²e1L?³îŽú'z£?ÙIn›5h?³îŽú'z£?ß´ R"?²8ƽΉ?àwø%¯Ö·?²8ƽΉ?¸)äOiW"?¼Cÿx×¾?ìúÃué™À?¼Cÿx×¾?¢3Š›àÞ?° |Ì¡ü?îÜÇV@S'?° |Ì¡ü?ÚzöŠx?¶ÜñMM?âÂõú:Ä?¶ÜñMM?º\Ø%Îú?£µHìã?ì¾4dûF!?£µHìãMIXED3FGL J1045.5-2335@pуùd@>à¼8*ùÀ:gK-û»ÎÀ;Æ¥®zÒ.¿ÑOƒ@r@
ö"»Á¸@ð¹@}ôx¿á»`…É$™¿ä½'J®¶¿çÈóœDnÅ¿åäS'¢FUNASNone@'ˆ¶+jçÕPowerLawnone?ïùºð<¤²?yÖ¢z@'?I>ÕYýÕ?yÖ¢z@'?ïלÆÂ-?ƒ=;·s™µ?t1œ—gE£?ƒ=;·s™µ?ï'\Ʉ˜Ö?‡KÚö}'?‹hÍ¥¹X?‡KÚö}'?ïîSÕÀ|?Ia\Æo7f?a¬)û7T'?Ia\Æo7f?ïá{fícµ?qôíÎNL?n"™ÝÛ?qôíÎNL?îúÙLâܯ?®*óa ©º? Rk1Ò5?®*óa ©º?î|'³1¬? Cw ®?¨?öÕ¨Ì9? Cw ®?î™Ä4!ð–?šcEI¶,w?¦c¼¾¼Ý¤?šcEI¶,wAGN3FGL J1047.8-3737@qW8›R~@3Á;ŸÀ:#`m(!‡À;­ÓÞ9Û¿ÖܙAÃ;@¸
n˜å?þR}`}ï?»ÀÝf‰2¿Úœ91$T¿Ë¬šlu¿çi øÈÿ
UNASNone@­s"FsØPowerLawnone?ïýƬnªÐ?1VÛj/¯×?1ʜÚí,ä?1VÛj/¯×?ïÐ%I­?ˆuåºxo$?wÿíiÝ	Í?ˆuåºxo$?ïØLJÇÕ?qÑs‹%Þ?sœ<†ÙD?qÑs‹%Þ?ïøbøGÏÍ?8êC¥N2?Nt¢Ñä?8êC¥N2?ïùá™?P¶áôìA'?K£'BD·'?P¶áôìA'?ï9ÐÁ›?°ƒ'ãù¬?ŸØßk6?°ƒ'ãù¬?ミ¬`È?ƒ°D;{N¨?€[ÔßbH?ƒ°D;{N¨?ïǐd‰?qί«ÌȀ?||7ähäâ?qί«ÌȀAGN3FGL J1048.8-5006@qºQc4'¿@ <½ý&À9ýýQÏÖmÀ;pŽÉ[ÿ¿ÖyÐä½@
@¶
Í@cƒ 3Ï¿ëhÝûÚh¿Ó4IèE=¿ã2>^4"°¿êÏYVTíºUNASNone@—³-\ú¬ÚPowerLawnone?í§$H<b?¹²w:bì"?²Çvݾí?¹²w:bì"?ï¯Îƒþt1?ø]v+3?"^øÓÏÂ?ø]v+3?íŒ`®kÃ?¢ED$>›?³œúŒ5žl?¢ED$>›?ïâä}Á?UüEå­8q?mü¶xH?UüEå­8q?ìw>?M?E?¸û}yeb)?¼F–Õ?¸û}yeb)?푿oŽz¤?»–?:00'?³rÔ\â?»–?:00'?êoZjHŒû?°'§»´X?ÆB–VÝÌ?°'§»´X?î#ÃsT,õ?ž½y\Í?­ÃÈÆq­±?ž½y\ÍAGN3FGL J1049.7+1548@luâlv@MÎ#žj¹²À:Ë*5]°À;Ò·£oÜ1?¹'ÄD©Wq@DÄyl'›@9Qx Ñ¿ÇD£¼ãýV2ø¶ò¿Ùô"U~{u¿íCWŒšUNASNone@›Ö)Çy¦µPowerLawnone?ï­ê‹‡?ŠùÍ!`—?"…]4È?ŠùÍ!`—?ïÛnêT®>?'»þýÛ:^?rHŠÈš\é?'»þýÛ:^?í¡2¥Í73?¡$žî2Ç)?²öjÒr-c?¡$žî2Ç)?ïÍ×)O¸-?^Ÿ÷úM¶?yk9çYÏ?^Ÿ÷úM¶?ï´eåq?…YªÈu@?'æ»Rª["?…YªÈu@?ïkáÇÓ
?§å%Lä?2ƒÏœ¤«?§å%Lä?íuséV?¤'¡©YE?´WÌhbÎ?¤'¡©YE?îE²(~Ú?›óVµh?«¤Ý{îT?›óVµhAGN3FGL J1050.4+0435@n±
gb@J´Ø]ú‡À8ê'"ÂÀÀ;s˜~§?ð%²úh¼W@ªð†y@ÂÆ ‹:Ü¿äæ}MŜ¿åmÏ557¿é¾Š¥ñþ¿èéM¯VUNASNone@'XiùrGPowerLawnone?ïþl$ˆþ?'š†¥û²ñ?)=½:fj¹?'š†¥û²ñ?ïÚ©h]{J?ƒC2>÷x¦?r«KØÑ~ì?ƒC2>÷x¦?ïÉÕo™Ò
?nX"¤³¶?{H»>?nX"¤³¶?ïö,í…?8ðæÝÅÙ?SǦwÁc?8ðæÝÅÙ?ïþn¶Ó!Œ?0U‡[R…å?)•{ÿ¥?0U‡[R…å?ï5&$??ª "‰ºGr?™]û@¥"?ª "‰ºGr?ï"Æ­gÆ}?†è§ffp?ŠÎT°]4Ì?†è§ffp?ïÜ<QSÉ?g¢¤¦,@?qáòÎgU?g¢¤¦,@AGN3FGL J1050.6-6112@r {5*"¿ú¹ýl§ÉÀ9gâTÀ:"Ö)làÔ?ñ^¦ß'mW@
á>µ[E@Ñ.à=B?ïþò7Y¿ëç…* åÔ¿ïÿí›ði?ïþ¾M¥UNASNone@ sU?|í'PowerLawnone?á,ýÙ¬{–?ÕýJ0ÙD]?ݦL§Ô?ÕýJ0ÙD]?îv;Åö;S?¿«üÞ1?¨œCžä|Ú?¿«üÞ1?æÓ"ãk?´ úD«á?ÒYº9)õÐ?´ úD«á?ïÑWY"W!?~Z:<¤?wTS.õ7¯?~Z:<¤?Üþªaà<8?ԅÚÇ®¢7?ဪÏáä?ԅÚÇ®¢7?å6±J˜Þ?ÒýþnÁé?ՒjÎCß?ÒýþnÁé?áÄÀS9/n?ºa÷´àz‡?ÜvY¡$?ºa÷´àz‡?ìr^Ð" G?ÄÈÊ\¨'?¼m	~êýÌ?ÄÈÊ\¨'MIXED3FGL J1051.0+5332@cUŁo@KÁÆ*\}À:{ˆe"¯OÀ<ñ¨Nh¿Î%+Ž@™ÿ¯Î@﹞¿ëvTÀ*æ¿áº—âÏ}¿ïÿ)Î'V¿ÜZN>–,–UNASNone@zGIã½PowerLawnone?ïþë'"P.?)U(UÏ?!MŒ'"›™?)U(UÏ?ïßIÚ²9?ƒw‹oçÀ?p[æX¯Z?ƒw‹oçÀ?ï˜O¤zj¢?ƒ¸r¹º-.?‰ìÝõ»š?ƒ¸r¹º-.?ï÷
Nž¯¿?@µ*pßÕ?QëbüYñN?@µ*pßÕ?ïûeyVƒ?Nkïy¤?Bj,¤I[?Nkïy¤?ï0ûi(žÁ?¨ìª'%G?™à'Þ[Ãà?¨ìª'%G?î҂ÔCí?›Jþåž?¢×ßö+])?›Jþåž?ï¶ò"'?˜pê2j3Æ?Ÿ‰!µè?˜pê2j3ÆAGN3FGL J1052.0+0816@n!ßzNz·@Lr)ZlÀ:{¨G²F9À;ã!"Î~~¿¦FéC\~@Í\%DÞ@ÉÇÿÞr¿ØçJÿz'¿è¤¢P¿åGrI7p¿´ÃÂV	¡UNASNone@™,<žíPowerLawnone?ïýáûu?9ð&?éGû?0ñãO9^?9ð&?éGû?ï܋ƒx½M?'Å:ŸGµJ?qº>C¡YE?'Å:ŸGµJ?ïœÇ>¡#?'ôí¸Îk?ˆÎ0JÇT?'ôí¸Îk?ïø‰úÉ?;ôU÷b?MØŽè?;ôU÷b?ïõD'M—Z?\xlúíø?Uv۱ȋ´?\xlúíø?ïQú|;?¬/¤-Re×?µÀ·WÕ?¬/¤-Re×?îµÌfµ? Ž\'—1?¤£?¾9"ª? Ž\'—1?ïj´_:?ÑÃ*sW?'½‰nñRÓ?ÑÃ*sWAGN3FGL J1054.2-3123@q7KƧïž@9'¹¾ÓÀ9ëUmßÀ;³'ìüíý?ëçBXÑ9@h|	泩@ÀÚñŒö¿ãFBÂGbÀ¿ëSVÞÖ\¿ç҆²X¤©¿ïþçSá©~UNASNone@zò䎊rPowerLawnone?ïÌ"|EÃ?{YpÙ
?yþµ§À'?{YpÙ
?î–溚×C?¢¹8½®N?¦'"W.r×?¢¹8½®N?ï( $Ö­?|Aa?šþ‹ö=Àr?|Aa?ìaaï´-?"¥™#ŸcÕ?¿ôð'^•?"¥™#ŸcÕ?שּׁ3$D®?‡%lDM— ?"Ôó:^p…?‡%lDM— ?ã­B‰×?ϽuÁÎ#?Ù¥ÿzìR?ϽuÁÎ#?ì_œD' ò?±`3Âf?½Ûvøt?±`3Âf?Ø惡Nˆ"?±%â(-å?㌾/X»·?±%â(-åMIXED3FGL J1054.7-6006@r
£Âˆ¿Ý'l¡"ãøÀ8…æ<à[À:7 Wù¼?æ¿M:ö@
Æ`Â7{@i³ +9?ï÷‡'að>¿êò1¡°¿å±ÊsbοáÉZ
§<´UNASNone@±GÈ}¿HPowerLawnone?ç2…–àà?ΫUók`æ?ÑýšôÒ>@?ΫUók`æ?îQú'LJ,?ºLÇ7U¾?ªàVÐóØ<?ºLÇ7U¾?åªb6»?¹H––HÆ?ÕÞ«:Œ‹?¹H––HÆ?î}|D@™?IJ²çÛ?¨(;º> g?IJ²çÛ?Ù¶")(K?Ðã"é [ï?ã$îëkڀ?Ðã"é [ï?ãº4h×?̏ÊÎDñ÷?؋ї.QÄ?̏ÊÎDñ÷?ãeÒÞQ?»xû$µ'P?Ù4[ÄC]Å?»xû$µ'P?ç
è™dž?·/€Ù×?Ñä.Í6ÃÐ?·/€Ù×MIXED3FGL J1057.6-4051@qŒ¨$x@1ÙUmÀ:yߙX+:À;Äîð
Cµ?äQSzW#@
êÖxF?ü#Ÿ—_ƒ¿ç	­³ø¿âkrÐé"T¿¿}t$¿þ¿ÁÁZà˜¨ûUNASNone@»^‰ã½PowerLawnone?ïþIYî¼i?&ÎxïÔtá?+j`ƒ·è?&ÎxïÔtá?ïĆ·ó?‰àBdBc—?}ót>Þi?‰àBdBc—?ïà=6¹œç?b–ˆ(Ä¢?oÂÉ*æ9"?b–ˆ(Ä¢?ïáâõy?T Ÿ/K@G?n1?Ñ?T Ÿ/K@G?ïù~ÁŽ~?IIJR$#K?Jû,Ýf©?IIJR$#K?îºyãñ­?¹§µf(Óß?®´Xe03?¹§µf(Óß?︠íÐl?¹ò4§ZÚ?×ÄÆBÂç?¹ò4§ZÚ?ïcáؼ^?‡hÍs|)?"ƒÄñEƒ?‡hÍs|)AGN3FGL J1057.7-6624@r>1[W>«À}'ÔÀ9«'!üÀ;<©Ôz@?Éþ"7ëÝ<@.®oês§@­-êñÑ¿ãG=Çå:¿êÌj¯ÔÌÿ¿Ö—¿s5W¿âÛמ%ß'UNASNone@'Ô~BZîcPowerLawnone?î¬Ñ«ó}*?ÀÆäQ4\?¥2å=X'l?ÀÆäQ4\?ï?b؁$Ç? ø0fšÖÀ?˜¤ìkË? ø0fšÖÀ?s¤?ŸÜå©.?§ô§,5ZX?ŸÜå©.?ïK"wÀÎ3?zè¯cÕÇX?–q¾Ïž?zè¯cÕÇX?ï=!ŒÓɧ?¥Bغ
Nê?˜[Îb/?¥Bغ
Nê?åŒàl&?ÌÔ×8Ç­å?Ôæ?á'³ß?ÌÔ×8Ç­å?ìýJ*ñpE?«0
‰Æ¾?¸®¨âqV?«0
‰Æ¾?é²ó*ë¢6?±®¬Uêàb?É43TQw'?±®¬UêàbAGN3FGL J1058.5-6106c@rœwškQ¿ò¨´wkÀ9&5îþÀ:HDK‰kN?ô—–"×h@E¬5¨ƒl@BÁf½y¿çZÙÀ¿ëûÑD¿ÝAåu´œ¿â_¥&À‰UNASNone@µx&Â&€PowerLawnone0?àùœ[c?Òu²?ßÜÇIç;?Òu²?éÿ½˜À"?ʲºÿè$Ž?È¥œÿw?ʲºÿè$Ž?æ
Gβ?¶Þ[Éu'?Óêåõpbœ?¶Þ[Éu'?ì¡ùšO?žúKÝ?º÷(3-‡€?žúKÝ?ÙÁb¸~X˜?ω,H!Eº?ãN£ÀÓ´?ω,H!Eº?ÌbÉô?̵ߙòÉ¥?èøç}
ƒ?̵ߙòÉ¥?äì§Ü[Ô?µ9t|_?Ö&°GIÚX?µ9t|_?ã¯ØøÕm?¾¨VJåV†?Ø NUÙ%?¾¨VJåV†MIXED3FGL J1059.3+0224@oY4Â@Jį¢ðZqÀ9˜ô¯úÀ;L"ø?Ûh_¤D1L@ªæÂAX@ÐßÀ‹¿´1]¥Í"ƒ¿ä¬ùAc¼W¿æÂ!=ƒ`¿é§"ü»kÀUNASNone@–ñüžì¿±PowerLawnone?ïÕÑE'k*?y(wÓ)<ú?u]Y—^ø?y(wÓ)<ú?ïÇ(A"ñ-?…û™ØF?|kßy†)~?…û™ØF?îá¼KÜ] ?•@È_9RZ?¡ä;B:&?•@È_9RZ?ï8æ"U·º?u|ØÀæW•?˜ã;³':Æ?u|ØÀæW•?îö§ª\-?¤Õßjë#? •…UóZ3?¤Õßjë#?íõiH:xÄ?³qOÀµüÌ?°Tµ¿ Ý?³qOÀµüÌ?ê›ðqÑ?±ÖdIWl?Ő>;¤ñ¼?±ÖdIWl?èDSÜ?°XæÌj`Î?ÍÃû¦î°'?°XæÌj`ÎAGN3FGL J1100.2-2044@pë•a'@A‰°¢ÊšÃÀ:H–ÂNĉÀ;Öu¼D¿M¿ï-Y[ÇO@þ\¿sÜ@MÅ¿g^‰¿íF½K¿É€tR8S¿ëA¤4Óp¿ÜdÌFÚUNASNone@Œ¬ÐbMÒòPowerLawnone?ïõïN	«Ù?cŽ,l‡J1?T!dO
£?cŽ,l‡J1?ïÛǧ|ŽÏ?'Ä«~fù?r,;‰LQ?'Ä«~fù?ïqr3?‡ÉXƒaºS?'ßQ»‡Ë©?‡ÉXƒaºS?ïÿ"‹¤?8ˆ˜Ü?ßírñgç?8ˆ˜Ü?ï–ÓâÑØ?'¶[cnO?ŠKK‰ýV?'¶[cnO?ï7[ÐKÝ?¬"Ëáz?™If Q?¬"Ëáz?î#e3Fº‹?¢6ú½ß?­É¬ÏóO?¢6ú½ß?ïᣙD_?k'Ãu
ó?n\êuÙèÀ?k'Ãu
óAGN3FGL J1101.3-6032@r²-V¿àS.øî¿À94íbnŠ!À:lÞÁÁÖпÓØe—^€ê@
°Øù‡Á?ÿu˾Úƶ?ïá…ï¡@¶¿éᖸ52‰¿âV?Zf†¿ça
˜¥UNASNone@Ã}v§ï²PowerLawnone?ï³t¶Ë?ŒºÊ"m<?ƒ"ü?êC[?ŒºÊ"m<?ïp¸ê—¸ï?¨Ž;ãhÂ?'èâ¦)ª0?¨Ž;ãhÂ?ëÌÌÒIÓ?­jôQR6?ÀÌÏÀ¶Ø³?­jôQR6?ïó.ðЯ}?G‹°dà€?Y¢ÙÖ?G‹°dà€?îÅø^îDc?¦öègw?£ z‹UÉ?¦öègw?ì1Û^#æ?ÅÞën‰±«?¿Žq%àÌ?ÅÞën‰±«?ë©l–3ç?­=×e§Û™?ÁZM§0c©?­=×e§Û™?ïƒÎ€£uÞ?'Ó¶½k,?_Éd¡?'Ó¶½k,AGN3FGL J1103.3+5239@c93Úøßz@LÀ!ÀD(NÀ:At™/À<¼²£V¿¿iòC÷%@µMBs@ñç_u0"¿à"°¦Ùý¿ê-	ﻐ¿åSÅÀÐ%ƒ¿ïþ'ÝQn!UNASNone@'>b¡µÇÎPowerLawnone?ïÔX¦yÙ?²é+NΟ?uÓ¬§HÇÛ?²é+NΟ?ïÞ8sÛ´?ƒ<#{·?pãûÀ'Æ.?ƒ<#{·?ï§A¹o2?{g¡Ê¡–—?†/' ÎW—?{g¡Ê¡–—?ïà6 óL‹?TàaÐÞh?oÉ_G̼î?TàaÐÞh?ïüªM?o÷ŒŽ ?;'­¯Wì}?o÷ŒŽ ?ï'-‰?§pЩy8?›lZNޓ?§pЩy8?ï'䫈%ö?‹…qp:
?FÕ!fp?‹…qp:
?î?cV«L8?œ²Ý2V²?¬	ʑ۠?œ²Ý2V²AGN3FGL J1104.3-7736c@r'—CécÜÀ/é‰XÙµéÀ9ul¡
ŸÀ;Qý¢W®=?ïd»þ8@O¥ 
Œv@_y5¿Ôpͼ¥§¿éM­TXê¿å_Xœ"ü¿ïÿGã<¦UNASNone@º
¸ºÇPowerLawnone!?î6>"ÂÎ?®Zéêñ¤=?¬œÇMÏ?®Zéêñ¤=?é7Ý¡}¶?ÀŠžž†z?Ë ‰z	'é?ÀŠžž†z?뺊RÝP0?¨·£~v‡Ú?ÁÖ´Š¿??¨·£~v‡Ú?èJtØ«9?¡\;F%sð?Î׺,S?¡\;F%sð?ê7X%â2?ÃÖiìáGâ?Ç"Ÿk"w7?ÃÖiìáGâ?Î/ôžfÌ­?ËH$؍±j?ètØfLÕ?ËH$؍±j?å¡w»g8?¸ºör£æ™?Ô½‰1Žæ?¸ºör£æ™?Ï7+e^~?¬‡»'X?è25&¨`\?¬‡»'XMIXED3FGL J1105.7+4427@dÕô!-w@OSS&ÂÀ:Ž=EíÀ<;tÈ)¿³"š²@
Îò+Öó@>Û_· –¿ã[ºæÆH¿æqrð§6T¿ä,OÖÏQ"¿à}J$þUNASNone@ŽfohÜPowerLawnone?ïüÓQeA?Kdøóé?9euÎÙÚa?Kdøóé?ï۞Û3(2?"ä#Ì%—?r0'KžóK?"ä#Ì%—?ï"!ÔLY0?‰Tc&¡ ?‹7Šìé³ô?‰Tc&¡ ?4™»¹?hÐÌÊ=7X?€Úف›^?hÐÌÊ=7X?ïÏMW÷Á?"•l%|˜*?xYT§{?"•l%|˜*?îeÈr ?µ Ñå±a?©£–K!
?µ Ñå±a?îæé—o)?›‡–}S"‡?¡'f‹£'i?›‡–}S"‡?êÉÌ`Úúý?¶äTžìÑ?ÄØÎ|"
?¶äTžìÑAGN3FGL J1106.6-1744@pçquŽ!–@C7-À:BHû"±À;¿~6fÄZ?õòs´@
2"a¤
@Bÿ¢7"?îmÇÆJ)¿Ð÷–±Õ¿ádZäªm¿ïäÈQ'ÃUNASNone@žÆ^ƒä%¯PowerLawnone?ÄÐG('!Y?ÄjNIÜd?êËî5Û·ª?ÄjNIÜd?Ç튚ֹ?É)€†<‰?êYJQ»?É)€†<‰?à‹Kù†Fß?µdË)HD?ÞéhórB?µdË)HD?Ó¶Ømûí?°øœ=Ë®?æ$¿É	?°øœ=Ë®?µF2.¨J?ºÙ7=P?íW9½ï§?ºÙ7=P?´«ŽW€?Àt<÷ÆåF?íjŒN5Ð?Àt<÷ÆåF?ÈZÏíœ-Ñ?³ç ¼c?ééL˜ôŒ?³ç ¼c?®5sk?–c»rNªr?î¨ãl)?–c»rNªrMIXED3FGL J1112.1+0500@orÓEŒÒ@LÎéd8À:T…òó¨À;À°',ãŽÀç§íå@:jôºL@¾ó ¡Ë?êÿßfWwá¿âóq@"õ¿èj~‹¿ÍRU`7UàUNASNone@¡»'E8ï5PowerLawnone?ïý˜lë2?>FNM/°g?7Ë=÷Ÿì?>FNM/°g?ïá%>¨Ý.?œE\=?nÚÁ7†i½?œE\=?ïð?e ?ƒ7÷ocT?‹Ãð7éƒð?ƒ7÷ocT?ïÿÿÝ£è0>tÇFl\p´>qpÓPïœ>tÇFl\p´?ïô¿§¦€?[?öl°»Ë?V€äqz/ã?[?öl°»Ë?ï^ñÆ	Þ?§'å¹\÷`?"!Ç9µºT?§'å¹\÷`?ó"?¡MÙêÀ[?¦d™bÎ?¡MÙêÀ[?ïÿõÞéÚÐ>æEFÙ±Zê>ÔB(ý?ß4>æEFÙ±ZêAGN3FGL J1112.1+1034@noY_í¦a@N¯hð"aúÀ:TËf›@À;Ë
Yö›¿´® HC@
ÙùXqQ@á'À8iÔ¿åK/99‰¿ì}0ÂÀ"j¿éÊãÙâ<©?áb$•ê;UNASNone@Ž
Øâe,PowerLawnone?ïþuÒÑ.í?.–\"l(Ï?(¢Ñp¢Ò.?.–\"l(Ï?ï߉Uu?'²+·"?p~;eúåH?'²+·"?ï°¶I[FU?{— "é¾?ƒÒmº€"?{— "é¾?ïÿ7¦[?ý¡Ò®R?ô¬«r?ý¡Ò®R?ïù:†4•?QßL~xHï?KçùxÚ?QßL~xHï?ïD'ÕU˜?§þ»}J?—mÅU_-?§þ»}J?îû´
Òë?—Ú›Âhż? O¤ÀڟJ?—Ú›Âhż?ïéZÚl´?nÓæ[é?f¥%'ƒtB?nÓæ[éAGN3FGL J1113.1-4515@qÕ¢£Y6@,z2	g‡ÏÀ:)ÆäUŽÀ;†N']‹?Í
Gö'¨Õ@
§ÍÓËD@–«ß—TÆ¿è2Ùhˆ÷Ø¿âÏnhF¿äT®€¨Ô¿å7&@l½ÕUNASNone@šXÇâ'APowerLawnone?ïû7JçQU?Jzš'ç¦i?C"Ô·d?o?Jzš'ç¦i?ﻌæ'Ö_?Š?S½\ ?ÆR;äk?Š?S½\ ?ï»{1,Pt?yҔ"¾qA?!3´;÷?yҔ"¾qA?ï°ãó/2?dº·ߔ?ƒÇ4ìßz?dº·ߔ?ïÀ'ékð?…$‰/ÎY?¶‹1ëô?…$‰/ÎY?íp˜}?»;—…Ã#?´{?ë—,?»;—…Ã#?›( A?Ÿ€S2¾)'?¦6vKÆ-õ?Ÿ€S2¾)'?ì1ƒ¥çZÃ?§¯ê¨z¿?¾sâÐÅ)ë?§¯ê¨z¿AGN3FGL J1115.0-0701@p'Â;yRÒ@HQt>–=ÅÀ9²!gXÔ­À;¥¥
æãÏÀóEâ¸Fƒ@ÛÄÞ@è~@ÞR 3Q;¿â¥ç*úˆ%¿äʑ5òÖ!¿ÛH´ª>†¿â§¡²AÜUNASNone@žk…S&ÂPowerLawnone?ïÿä1z>åö×ێ'&>ëÏ\SP>åö×ێ'&?ïßfó~?°|uΎ›?pLñ§x¤?°|uΎ›?ïö¤"Dߔ?X[1¬Ž?R·»?—…?X[1¬Ž?ïÿÿãKè>q"šÜž>lë*¾¯ Ì>q"šÜž?ïÿéä×ýÐ>âQd)4>ææS"³r>âQd)4?ïO®ø;³?ª§Òӈ?–
<ÿ@»¨?ª§Òӈ?ïøœn‹#	?]Øýúm¢ ?MŽEiY…?]Øýúm¢ ?ïÿüÒ£üI>Ã¥ªD«>¹k›'b«>Ã¥ªD«AGN3FGL J1116.7-4854@qõ>"åÞ@&)÷LsÀ9ÑûÊçÀ;veŒKÓ=?壪¬2ð»@—k0O©@­J 4¨Ô¿ã°ÝŒ§\•¿ç·ó…âòB¿ê&µ×›e¿á³
¶w½UNASNone@Œ£ÔɅðoPowerLawnone?ïý£òc	e?4¬€BŒŸ™?2àmÀ¶?4¬€BŒŸ™?ï˜'	R9?š_öêëa\?‰þÛ¶Ì9½?š_öêëa\?ïÎÉYµu?qLŒ\"@?x›sÁ÷9f?qLŒ\"@?ï—´ƒf
?jç$.³r?Š:'Ôרá?jç$.³r?ïõ²ÙR?Z›˜Ê5ý?T›ÐȳLC?Z›˜Ê5ý?ìK2À"ûÂ?À†"ÄP?½¦iû`!í?À†"ÄP?ï2ãÿ2>…?",Jxٌw?™£€ÅZ?",Jxٌw?ëΰ=õÚ?«Y+"+Á?ÀÇí?(˜?«Y+"+ÁAGN3FGL J1117.2-5338@r,\ý
@¸èBt×À9_Çȁ
²À;aHZ⤥?ϟNéÆO@Ô>¢ýñ]@uÿ‹í¿å2. ­R<¿Ü<
"¦¿ÓÒ×CÚ['¿â]֘[3¶UNASNone@¦P}p£×
PowerLawnone?ïýt¢
β?.fO{ô©i?4Zï¯	Ì<?.fO{ô©i?ïª==£#±?'¦C§óÅ!?…p°Œè?Ì?'¦C§óÅ!?ïæöښô@?g	d"Ùd±?i	%`ì7Ï?g	d"Ùd±?ïí·!%$ä?C¡Ï2ª?bHÞó˜L?C¡Ï2ª?ïûŸBÐà?<Ä­¡Ñlš?A'õtJ½?<Ä­¡Ñlš?í¡Fmü_?¾‡Çcp+¦?²õ̗À?¾‡Çcp+¦?ïÄ|@î1Ì?ƒ–Çõ¨Y?}Áß~˜Eã?ƒ–Çõ¨Y?ï˜Ô¸dÇ?vD.§4E?‰øŠÎw2A?vD.§4EAGN3FGL J1117.7+0217@p
Ô`ªdÃ@LDêòRÀ:0ªRNmÀ;ʤŠŽcÛ?××2lõÝÎ@îáI±z@9è_ÐJ0¿ÂOØÊã¿äÙGdÌ¿ä"ùiÓÈ¿ßþA†TÇUNASNone@™ÕU›=ÈPowerLawnone?ïý9f©l?Q!F\ìÑ5?64ÊoÊä?Q!F\ìÑ5?ïÖٗ¥<?ƒÐñc¶ê?t"4uDÃ?ƒÐñc¶ê?ï¿(Þ+Ö?l˜WÒ?€5ȂÈï3?l˜WÒ?ïÖÇ3½G?W*t¢Þ«?tœq䘟?W*t¢Þ«?ïûþ‰ïh¿?C.ùæ'6?@Ù>&Çÿ?C.ùæ'6?îãªåx,?¬à,&ÙÆv?¡ÅQ¯$dF?¬à,&ÙÆv?ïˆq/qC?‹~ŒLÇ?ã Aâ0?‹~ŒLÇ?îFͧƶ'?švR)³üž?«"%"p}ò?švR)³üžAGN3FGL J1119.8-2647@qmMüã@?ÂÚ/­mÀ:j<?KojÀ;ñÅ	‰ì¿ÆÔ_ï @ì;›ât)?ýSwê"¿í\B_[ö¿æ&+7]±®?ÙûHñÓ¿ãZG'öjUNASNone@²¤Í'hr°PowerLawnone?ïÿËâ
ž?a½ˆ¥{?Í
´ÊÓ?a½ˆ¥{?ïÚÞu°u?ƒ+ÝÝ¢ÿ:?rþÕ¥å^?ƒ+ÝÝ¢ÿ:?ïðáž.îo?`àӃ¹ø#?^<Ã{§'œ?`àӃ¹ø#?ïþà<œ? 2Jñ©6?.ü{Q­Y? 2Jñ©6?ïÿ ¬%?Ö-<wY?ú†'¾S£?Ö-<wY?ï,fB+"?¬ÕÚÁÆÎ?šs7®bÁ{?¬ÕÚÁÆÎ?ïñ"Е?gëè WÃÊ?\÷ܱK…ó?gëè WÃÊ?ïù@Xé-ß?MFLed@?Jþ›ê—€?MFLed@AGN3FGL J1123.3-2529@qpö@c^@@¡˜¿pÀ:$€èȬÀ;ȯf•¿«¬"'µþ@kÚÔ¢Y1@Líõ®˜?ë+Uæïì¿çÙi‰9²¿Ø΂‰ÝŽç¿éxuäw})UNASNone@'áY‡+PowerLawnone?ïúc\ào†?G"92ð?Fr‹v_êŒ?G"92ð?ïÓK"EÂ?"0§Çí…?vZ}ElC?"0§Çí…?ït%Ö="?‹âM™!?'{E@‡÷´?‹âM™!?ïÕX_ù ü?^'²À]?uSÐmQª?^'²À]?ïôÜY1Ê?YS:øÁø©?WGÌ
V?YS:øÁø©?îöcmöÇ?­)Ë}ÝÊx? ™É/Øa‹?­)Ë}ÝÊx?îÒÉ24?™Àñ³rCû?¢ÓnrѾ?™Àñ³rCû?"œ»ž?•.òJ¤'Æ?¥vöÅX_?•.òJ¤'ÆAGN3FGL J1123.6-4558@qö5ü;Oa@,y‰7KƨÀ:1íÚcŽEÀ;šsîå%‰¿mYñäv‰@º\JØw@Žc|?ïýFýå¿à¹f™ù!%¿ë\D¸Ü³?°â×Ö¢*æUNASNone@ž©xÔýôPowerLawnone?ïéâ1bùt?{¡Q—ú?fÎ|
K¸?{¡Q—ú?ïÅ"—ëªÅ?Šæè+ø×B?}n´‰5Ÿ?Šæè+ø×B?îô§Å	?"¤‹þ

s? ¾…‡úñß?"¤‹þ

s?ïó°2úd?N@ˆq®7?XŸç÷€–?N@ˆq®7?ïšÐƒï?'ØV}A¡?‰Kß:á?'ØV}A¡?îŸkK?Ž?´UËi+"ì?¦	KP‡î&?´UËi+"ì?íF5)¾¦?©âqHÉpÂ?·ÎV²
Ì?©âqHÉpÂ?îõa
Œ±?¡K¶•[z? ©ï)Óió?¡K¶•[zAGN3FGL J1125.1-5803@r;N…3±@S¼Œã©À:RT`ªeÀ;9,G†§O?åu5¯—æD@
↏-?þw€?*¿ïìꏈý?ä<aëyÙ?™©¤/ó¿ÜêUU¿FŸUNASNone@ÀÙ©ûçmPowerLawnone?ïúõ…ŽÛâ?Fš:h=ú?D)êÇÔÖ?Fš:h=ú?ï7ð¸Æ?©zn‰Š'Ã?™éEQ.?©zn‰Š'Ã?ï¼	ÌBÊ?ìü'?€ÿýmmP?ìü'?ïˆÞi

S?r~Æ"Dh²?Èe½|«U?r~Æ"Dh²?ïí'?^j¾Œ°Ž'?b}ò	¢_?^j¾Œ°Ž'?é·3dþ©¶?É«9X€
›?É#2lY(?É«9X€
›?ïwf
î=?ŒY3¾ò?'s@Z]?ŒY3¾ò?î'Wד‹?š…¤âÈÄ?¦îڄ>•F?š…¤âÈÄAGN3FGL J1126.8-5001@rҝÇ%Ä@%1uÀv}5À9¢V[LÀ;Œ•ÚÈ8?â£ë#î^@
 úS˜®b@ht`O $¿èµBÙ¿àÑ3cښì¿èAÌsê2¿é¨ó8hɏUNASNone@‰!–R½<PowerLawnone?ïä¼Î?§J>§*ˆ?œŸƒfÇø6?§J>§*ˆ?îTÀ€Û?­ÍoWMZ+?ª³÷ôÛÄ?­ÍoWMZ+?ïóxï;H?'nâlä]L?ŸÁà`É?'nâlä]L?ì½¾Bõ??'ÊE?™´?ºeèV?'ÊE?™´?æ	¸"pÃ7?˖zµþª?Ó쏻y"?˖zµþª?ßféª9`?ÑVhðŒù?àp̋*ãP?ÑVhðŒù?é»dÄó?³³'[Ïå?Élì3ç°?³³'[Ïå?ÕÆ~¯]{0?±jO•½?åÀ¨QBh?±jO•½MIXED3FGL J1129.0+3758@eõ5¨Xy>@Qf&,ºs.À9€E¯6¹ÐÀ;|išÎM?î6oùÀ©\@h¬¯Kº@N•`Nõ1¿·ÇúË¥À¿äÑ/÷®<¿áú6Æv؋¿ìuƼEÊUNASNone@™Lˬq³PowerLawnone?ê¦Ø¨3v‹?ÁiÜõ[X¹?Åd_2%Ó?ÁiÜõ[X¹?ë`œ¬W?À0Àè"—?Â}¯­N¥?À0Àè"—?ê}jš*A?¯&YzØ~Ö?Æ
WŗVý?¯&YzØ~Ö?çø1O¶Õ?¢´(¶Že?Н`'UÇ?¢´(¶Že?ᜃç*Æþ?ËÇVû(C°?ÜÆø1ªr?ËÇVû(C°?àÇZ‹MÞ?ÑUyÉðyz?ÞqJéeèE?ÑUyÉðyz?ॸ}NN0?ÀñŽòo"?Þ´ccŸ?ÀñŽòo"?ͯíù˜1æ?«ïKR1?è"™ó‡?«ïKR1MIXED3FGL J1130.7-7800@rª"záG®À/ 0 ±»ÏÀ9è<ʋ©íÀ;ƒÀü´ñå?ëe-žÉ¯6@½~Õ(Z?ûØ€nz\¿ï±Â¦"e?åv´@;¿¥šŒéÊîØ¿ÒùHápGçUNASNone@·†°¾
í)PowerLawnone?ïðM:Îæ‹?]ÚQ`•úý?_eŠ>vú?]ÚQ`•úý?ïŠnîË$V?¶uyR?dDFW²?¶uyR?ï¯ÁdA{©?í«É*ك?"¦èÁÝÌ?í«É*ك?ïŽÌä6ð?m¬¡Á´R?ŒLÇÁÓ?m¬¡Á´R?ïÚû=šâ'?q˜ÅÁӐ?r'aRÛ*?q˜ÅÁӐ?ëòêg߯ ?Ãù/ó'?À4V`A€?Ãù/ó'?ï,Vª-?•3Ä\ù›±?šu<IÌ[?•3Ä\ù›±?î½fâÚw¨?'R¨¨º¦?¤)'Îèé‹?'R¨¨º¦AGN3FGL J1132.0-4736@rZ¬1@*SQÞïåÀ: @‹áJÀ;´)Žnÿãê*ÍB>@±§+'¡@韍#•¿ïþž-Ò÷?ïÝ[Qy36¿à¬¤±®@ù¿æ3²UìàWUNASNone@¡$+…¸RPowerLawnone?ïýn²²'°?3væÄv8U?4Šj»¶/÷?3væÄv8U?ïř†ñ˜«?‰.Ø@Úvë?}3<f7jn?‰.Ø@Úvë?ïÌ )–&s?sê™ÕiT‰?yïëUé?sê™ÕiT‰?ïæ_+ÎSÏ?[ÇK%Ϟ?i ÔB*Pš?[ÇK%Ϟ?ïöèHö‹Z?RVâ`m-?R/nR"š?RVâ`m-?È7ã?´Ý4#ù"y?§UóþÆ?´Ý4#ù"y?ï£ãC©Œ?"¯
1˜½?‡/#xÿ?"¯
1˜½?îKuwƒø¦?£9°__µ=?«H¨‰xC›?£9°__µ=AGN3FGL J1139.0-6244@rkî¢	ª¤¿ðZ*~…À8%ô¬å§À:…"_u±]?íä+¬3ب@·õ$YÒ@2^ÿê±d¿ÜSä,©›¿â$ËdÓûP¿ã1O¬Té¿êc€ò†UNASNone@—¯4Ö¡bPowerLawnone?Ñç"ìò?Ïwx£fW?ç}n‰†¸?Ïwx£fW?ÆVë`Ù.?Åm^'²t²?êjE'É¿ô?Åm^'²t²?抬egý"?µuŸ76¹?Òê§50ø?µuŸ76¹?ÛÃPÂe?Ë?¬/
™!¢Þ?âWžÍ`?¬/
™!¢Þ?¦à¶3)?°FËv£"Ü?î'ôŸ#Ç/?°FËv£"Ü?˜òWÞ©½*?°øqÔHí?ï8mAp‡?°øqÔHí?Òî÷2ë©v?º"áÈÿ°?戄fŠ+E?º"áÈÿ°?ªhŸHï®?œÀ
ÎT?îYFBjÅ?œÀ
ÎTMIXED3FGL J1142.1-6941@r\|ؙÀ}¾Ý 'À9¾±û.·À;:Æ/#Ú¿Ú®ÛÌ*K¿@ÝX›L¢@F˜ÿÀ¿ù¿ÝnŸ+:&©¿è槍çÎu¿è(Aš Ÿ¿èŸÈ,¨LUNASNone@‡qv+jçÕPowerLawnone?ïõHZÑv™?VÙo…W?UoJ(ؽL?VÙo…W?ï¦A&œÍ?'ãþ-É»?†o¹€§ ¼?'ãþ-É»?ïu­Aí
?‡Å¸­òFM?'^*Yz,²?‡Å¸­òFM?ïø|Wáµ´?6×ÈÍwé?NŸi"?6×ÈÍwé?ïÓLuEô£?€C›è™Ö?vYÅ<	n‡?€C›è™Ö?í*vÂePù?Àoé¸ÑÿM?¶¬Iìg"º?Àoé¸ÑÿM?îˆì€ÏÒ?¢NuV^Õz?¯×q4ƒfé?¢NuV^Õz?h5ڔ?~ift à9?ŒŸeäÊë,?~ift à9AGN3FGL J1146.1-0640@q8Œ½D¦@JWe<š»À:EFšï/À;¼ì÷À?å×r%?Z@éeß­Ð?þ»È?õ8|¿îZÖ×"ø9?ÉxLÞ¼»¿Èܸûè ï¿å 5j%UNASNone@­Må`A‰PowerLawnone?ïýš"?0ݍ÷Ïìa?30æîî‰?0ݍ÷Ïìa?ïM.|ȱ?•'úiõ?–Z0lG¼?•'úiõ?ïÙãµæ?g-ÉKiß
?s% ¹ ?g-ÉKiß
?í¼³Ó½½÷?'ˆX(¶¯?²aa¤Æ?'ˆX(¶¯?ïñX¾Lµ?]²³wiƒ?]NäàÛõ¤?]²³wiƒ?é6µ…w<'?Å~¹›	•?Ë%)ê#
»?Å~¹›	•?ïªeŒÕCœ?'´ªՋÁ?…fœ¼ð¨ø?'´ªՋÁ?äòJæRì?½5g•æ\?Öj3ûZ)?½5g•æ\AGN3FGL J1149.1+2815@i•nÖwpz@S¤i×4/À:JÊ<ϔ'À;Ï#K^£$¿ÎþŽ]GÑ@¨¹ù¶dÖ@©¶àQcö¿ëÂ`?äO¿ã~œbC8†¿ÞôRds>ˆ¿ä®àc隟UNASNone@‡å	 'RTPowerLawnone?ïÿ3
ž?
õ­á»Ù?û$%$-?
õ­á»Ù?ïálóã?'»cSƀt?n" $7?'»cSƀt?ïàêöAÄ?f‡G\'Ó?oùՄ,{?f‡G\'Ó?ïóÂ
2ê?A‹-ä nA?X{ê áü#?A‹-ä nA?ïþó·¶ÿË?*´5Œ:? āx]XO?*´5Œ:?ïFéÞ-•?¤é)¸€Òˆ?—"ßk…`?¤é)¸€Òˆ?ïŸí+o£?ˆ	 E¯?ˆµ$??ˆ	 E¯?ï\OH‰þé?‰!"ˆcŠ?"víTÙ?‰!"ˆcŠAGN3FGL J1150.7-4816@rIø -à@*½½×fƒÃÀ:Xóz¶ƒÀ;¼ AS‡g¿Â
ÎʨÛ+@ùÔLfá@¢ÿZcN?Üù)Ƒ¹¿åՍÌÂø¿ìÛ·ÿ¾Å+¿¹Œoôág.UNASNone@"IÐbMÒòPowerLawnone?ïë
¾cÂ?‡íZÔuå?doõs…?‡íZÔuå?ïĬɬ~?Šn'Sš?}©ò|Tý?Šn'Sš?î«ƌí?˜¯«&za?¥N_7Í0?˜¯«&za?ïô…Sot?Hå4[mz¢?VõY^B6û?Hå4[mz¢?ïF
ß¾'T?ÿ•.Í^G?—>£ÿ¤"?ÿ•.Í^G?îa=ÌX"?³ä³"2®?§	ì$då?³ä³"2®?ëÔÕ±ð?±~I'¼±?À¬©8?ƒñ?±~I'¼±?îͤWQY?¡íÇ»ž…?£%ºŠ#x?¡íÇ»ž…AGN3FGL J1151.5+0957@pJ^~¥øM@PñŠÚ¹õZÀ:|ـ9vCÀ;âÍ)Á¿ö­sU¸`@¾_ ø@Ŝ@Ô¿ßےêË1ä¿æ)jÀúAá¿Ü¡ú¤t¿è‰¼qOUNASNone@˜×›ô‡ü¹PowerLawnone?ïþå¶}ªü? xýWaù?!¤—–`‡[? xýWaù?ïâô÷ÿ?æx³G!?mç'ÐÂ?æx³G!?ïáË7)ª?kÇwRèÊJ?n4ÈÑkö$?kÇwRèÊJ?ïÿ Þÿ¡®>þ2Ì
—ý…?È<Ìùr>þ2Ì
—ý…?ïþ°
	¹ù?$#4‹øL?$ÿ+]ä_?$#4‹øL?ïi`ùŒjÔ?¡Ñð2x?'ÓàÎr¥u?¡Ñð2x?ï´SÊ–X?ƒDX?'ë
|'Ãý?ƒDX?ïöÉ»ä·?RZˆ;=7Ø?Rmè('µ?RZˆ;=7ØAGN3FGL J1151.8-6108@r|Щ*0?ìʏ۪¶"À9	ï]ñLßÀ:ÒFfޏ?êZz%q9å@ðé‡B©ô@w†ß­¥¿Û?€UrD¸¿¯;!îV#<¿ë#Â2G®s¿íÔەx³×UNASNone@Ÿ`ù	kºPowerLawnone?¼ú"s ?ÁŽ¿¬±W?ì|?à¯qŒ?ÁŽ¿¬±W?è\dT"U2?Ækù€è{]?Ύn­²«8?Ækù€è{]?ã"BN¦x?³¼Æ…»	?Ø×{b³Ç?³¼Æ…»	?è˞­Ø'?£

Q ?ÌхI¼¼?£

Q ?"Ä-¦]K? ÅÑ÷R33?ï_ޅ¦? ÅÑ÷R33?ÈWH't?Äl;Œ/?éê-ÿbú?Äl;Œ/?Ñx婃¢?¶%›ö	??çC+¾/?¶%›ö	??Ì7`Ћ"?­û{sÚ;w?èûr'ËÝ?­û{sÚ;wMIXED3FGL J1155.3-1112@q˜|ßýa@H©>¢Òþ?À:ŽK†ýÀ;£1ßÈR?ð
ƒ® ¼Î@`þWN?øIúÑÃ?é#ÛΌ.f?ëšG>'ó?ç(fº¿ß/DÜRü§UNASNone@¾¦g®záPowerLawnone?ïð"i~Q?bKب›"?^÷-i‰ÍD?bKب›"?îä«î'\Þ?¯Ô!©Ën?¡µA!Õµ ?¯Ô!©Ën?ïJ5˜¾'n?dÛQúÖ?–¹LæƒDR?dÛQúÖ?îߜ_òƒì?–z£Úò?¢:³¨F?–z£Úò?ïæŠlľ$?olÈì¼­?iu"5Â{°?olÈì¼­?ìþ&ª—K?¯x¤½ E?¸&ˇ,¤?¯x¤½ E?î«aiýJ?I^'?¥Nëùa?I^'?îÍp,'D?©ñžnc·•?£(ý@±@Â?©ñžnc·•AGN3FGL J1200.4+0202@q-¼U†D@Oq²•êÀ9ã£v'-•À;¸îA'šÈ?ß	袧pƒ@#æ9/w@H½§Õò¿çEÂ[H"Þ¿Õv.­3÷¡¿Ôc)ÖÖ2¿ç¼*¥ðêäUNASNone@ 12-VPowerLawnone?ïü¶¨s&?BG .¿Û??ÊK:Ømf?BG .¿Û?ïÎg$/ï?"¸iœ‰Ö?xÌmïV@}?"¸iœ‰Ö?ïä͑¼Ì?fÙ	'Œ¬?k2nöƒƒ›?fÙ	'Œ¬?ï…͏Èèð?ná€úðƒW?ŽŒœ—é?ná€úðƒW?ïð½mféL?`#›Rcʊ?^…$굈ë?`#›Rcʊ?ît­Oj1³?±Þ(TMr?¨µ+
¨gÆ?±Þ(TMr?ïÁÂÝÍü?woWÍ?÷0µiÙ?woWÍ?ì¼ek¿–®?¥öa2ÚN¿?ºÔ¢J?¥öa2ÚN¿AGN3FGL J1200.9-1432@qÐVÕϪÎ@GHw…À:NÌ7«hÀ;¶­¦–Ø?Ãwx'7ûo@ø,*€\1@)«0ñ¿íŽä["ª>¿ÜI6¶† ¿ÎßÎÅ~–¿âVÎÜz"UNASNone@˜•—§†Â'PowerLawnone?ïþ'¥{Çn?$Ã)	Ú±¡?&å¨~èÅk?$Ã)	Ú±¡?ï×ÔSe?ƒ¢Ý8ï—?tÖAÇËÞ?ƒ¢Ý8ï—?ïÏïôf'&?{ž–;¿Áp?xâå?{ž–;¿Áp?ïò`°ì?@Ó.†hHñ?[>Ÿ¡ë'¤?@Ó.†hHñ?ïüB˜×?CP¶)JR(??¥éï×m­?CP¶)JR(?ï.TQ;?®Ï@=´uÑ?žš5yH;9?®Ï@=´uÑ?ïL•·Y?"?•r‰N6³Š?–mI°¥Ž?•r‰N6³Š?免âÒþ?x˜½‰…?…ÓGNî܉?x˜½‰…AGN3FGL J1203.9-1745@qó\=îx@EÓÊ}g3ìÀ:R·*¤yÀ;ק jٓ?éð¸Á^ã@ù½',±@ZH@5¥(?ág6s|¿Ï¡ò3Â-¿âýÕÊ2¤Ô¿ïÿ'wJUNASNone@šYJôñPowerLawnone?ïögŒ'?©±|êU?Ÿ3¥9»?©±|êU?íÄ¢"hR?®>²X²gª?±ß2êâñ?®>²X²gª?ë'wEåE?©ª)%;™v?Ãb"èjë?©ª)%;™v?êÇÎýð? "Z	ƒ?ÄàÄÄ?œ? "Z	ƒ?îK×gc3?±t^¥ì}?«B‰>Ó?±t^¥ì}?åæ(	g?ÉÀ`öÃsæ?Ô2߯í1á?ÉÀ`öÃsæ?çמö3ê?´½¡W(0?ÐPÂx"˜+?´½¡W(0?Ø3†¤8Gß?´Áuø÷ð^?ãæ<­ãÜ?´Áuø÷ð^MIXED3FGL J1205.9+3315@fGohی@S›Då^³À:WÌ¥_ À;èÚ'QU?ä¿ÃôOâZ@
þƯâÜ@·9_‰¿íøÔÔy@¿ÞòÇK;¿äÕxÔ
o¿Óý™üÉrXUNASNone@"Iþ†ƒ<PowerLawnone?ïþ³ô'žn?-¿{›ûËG?$ÀÁäH§?-¿{›ûËG?ïÑY¸ÇËö?…Ãi$E?wS#—ú}?…Ãi$E?︴5•ýÈ?|ïvP¯g?Òòœ8\?|ïvP¯g?ïy ƒ5ݐ?wWÒú	X0?Ûïžk·õ?wWÒú	X0?ïùµN3D?V<¹á7?I*Æ%C?V<¹á7?íŽ
¯ô'|?½D)"gÅP?³'€Éß ?½D)"gÅP?îÔ"¤¦Ø?˜²"f,:ä?¢¾¶ÄÙ«†?˜²"f,:ä?ê¯ÆÑ$A?µÔS¹'¹?Å@ä»oÆü?µÔS¹'¹AGN3FGL J1206.4-7123@rµ7KƧðÀ!®ªm&tÀ9ƒ@ìYZÀ;k8$3»ï?ê'~~@%¤ÝD"/@qM éÀ¿è'½{ºÐ:¿é8úž}jJ¿åÚ´¼Dñ¿ïÿ¹ý£jUNASNone@~~²¿ÛLÂPowerLawnone	?î5UA…?²x"²î?®Œª±œ¥?²x"²î?æþ~KƎ+?ÅU1à¢Â?Òhrã«?ÅU1à¢Â?í~÷E,–?¢;"ðVX–?´E×	B?¢;"ðVX–?èDmŸ?£*Ž¢YV"?ÎîK³Ã͆?£*Ž¢YV"?êwLl"8?Æ¥4~"Œ?Æ"ÎOów?Æ¥4~"Œ?Á
Ïøâe¢?Å"¤
ÇëM?ë½LÇf˜?Å"¤
ÇëM?ç]î	³]?¸ÈZxō?ÑEà#ì™F?¸ÈZxō?Èغ£¡Ò›?ª8üÚ]cp?éÉÑW‹Y?ª8üÚ]cpMIXED3FGL J1208.0-6901@r°µ^ñýßÀíäßé	CÀ9Úe;ÃûÀ;hK!f'?ç'͌\½@
¾öJt˜@ÞÛÿo·H¿ç¦2™°?οã/žùÅ¿åÙx(¨F¿ïÿíK¥ùWUNASNone@ˆ5?|í'PowerLawnone?í'Í×R¦…?µØ½Ê?³q'EØ¿Y?µØ½Ê?æÇ÷ª‹?ÅÂøzGW?Òqïôªê?ÅÂøzGW?ì	'¾Wa?¦‹€¾`¶??¿§¶Â
Dü?¦‹€¾`¶??çõJò<?£[¤º‹¶ë?Ðkú†ç?£[¤º‹¶ë?ã
¨;ÀAñ?Ïýý=Ð<?Ù䯈|?Ïýý=Ð<?¾'«O	å?Â	òÿÞ¿`?ì>
ª–Ã?Â	òÿÞ¿`?åøE¡u?·lؔ'ä?Õÿàt½?·lؔ'ä?žOއÝ?§0pxG–@?êl^?É?§0pxG–@MIXED3FGL J1209.9+7607@_Œìk΅4@D^™côÏÀ:J¹¥¨œÀ<{DD¿Ó4ƒÄ‰öþ@
§ÑjÁ?@/`œwð¿å–âcâÓ¿èësg<¿Ñ'Û ïÜ¿í>vÒçjUNASNone@\šu%FPowerLawnone?ïßXê€?wÔorä¯?pS÷øl\M?wÔorä¯?ïØÇY›QÖ?ƒ+©$(ˆ?sœSQC'?ƒ+©$(ˆ?îÌØnÒ¬Ç?"'Ø=¬'?£2ye——?"'Ø=¬'?ïàåGçº?XÚè!ɟ¸?o¹51[?XÚè!ɟ¸?ïi‹6Z?Ÿ…«Ê}²?'Îœ´êÕ?Ÿ…«Ê}²?î±mNùQ?°ÐGoov?¤é/éXœð?°ÐGoov?íÍØl­?¨TØO<?±—§`³š?¨TØO<?†èÖ²?žk.Bv?¦ôW'r"Ù?žk.BvAGN3FGL J1210.1-2742@r>ýuâ@A"–'§\ÑÀ9©±¿*À;€8YáÀÔ7cnU@ë&šž|W@¾Ç :ˆ¿ç­U™c¿ê]hÓþð6¿ØR×	Þób¿êà‡Q:UNASNone@…F%`A‰7PowerLawnone?ïþ¸—¶•~?9ÇÈÀi°u?$v…ÀԎ?9ÇÈÀi°u?ïÝ%Jq?'¬Ÿ¿ù?qm[ä¡?'¬Ÿ¿ù?!wZ;?'€>«k¼?‹\·¯çá<?'€>«k¼?ïÿÿµ_üH>†–hÑÈ!>'¡¤¥t_>†–hÑÈ!?ïÿÁ*σÙ?ïVÆñœ‹>ÿj{ü+{?ïVÆñœ‹?ïEŒTjC?«ÌN&ól›?—NutojP?«ÌN&ól›?ïÓpoŽ?€3¥%>U?vGú;*-'?€3¥%>U?ïÿù­Þþ†>Ðî\_‡½[>ÉGÕîb>Ðî\_‡½[AGN3FGL J1211.8+6413@`>ŒSâÖ@J.VCæÀ:Ì-–;@HÀ<3¢¾‰­¿–Ü,ïªÑ@
%›@xqû¿í¶âyÔ¤ª¿ÉƒËÒ{¿æُŒê"¿ÜœVH9UNASNone@lQ'©"PowerLawnone?ﵗcßMƒ?"ëâÒø©Ø?'š'cÍ;?"ëâÒø©Ø?ïÜå‹àss?"Hµè?q:0†s?"Hµè?îµåp˜Õ‹?›I'9‡‰l?¤¡¨ó[?›I'9‡‰l?ïáõ©öð?VsüÆ¡yâ?n
UÚU3'?VsüÆ¡yâ?íÓµuÜêÁ?·™®û7ì?±bTO`Ûû?·™®û7ì?îÕÊ>t|K?°¡8€lOs?¢£\'×I?°¡8€lOs?ìѨ¾D?©ýÁh=÷Ÿ?¹rº£^?©ýÁh=÷Ÿ?íÞ®Û…â?¤í>0³?±
‰'ÓÐï?¤í>0³AGN3FGL J1213.9-4412@r~Â&€@2$Wâ?$ÙÀ9›Õ¹ÛÀ;"«² Ñœ?¤63©åv@üW-
E@'§_ÕӇ¿Öaé0¨
î¿æázéÞ´¿àsHš(½¿é}œ/mxUNASNone@'½âMÒñªPowerLawnone?ïö+bPÏs?WÖs`±±?S©;¶W?WÖs`±±?ïÆÚêi7I?ˆé®É›XÐ?|'ŠØrߧ?ˆé®É›XÐ?ï«{ɤú ?'¢';¬S†?…!
š1?'¢';¬S†?ïÁCÌTú%?b+aw¨#é?^ÍCÝ«?b+aw¨#é?ïÑ0¦)äš?{Y"ûä?wg¬Ýÿ/7?{Y"ûä?îbmé›Q?´ñë‡ég?©Ù!g*qô?´ñë‡ég?îªÇ°ÇøA?œj"w+W2?¥S"õ8Iõ?œj"w+W2?í=¥è°? ØK«Ü¥?¶zÙ"þ? ØK«Ü¥AGN3FGL J1214.4-2315@r?÷eýŠÛ@Ci/Âej¾À9õÅGMƒÀ;šñ,'¦7¿ÝöECM@

ÛF["@‡Ÿœ¿äšgãq²}¿ç¨ýÀ	ÅÒ¿âB`m†žÉ¿à5\ë_×MUNASNone@'¸FYJôñPowerLawnone?ïýÉARÛ?3åyÈÓ³u?1µöj‰wG?3åyÈÓ³u?ïØÞïË:¸?ƒCÄÿç"ï?sˆ4¬
?ƒCÄÿç"ï?ïÆ	'Ïã?~T÷^áÚ?|û7	QÆp?~T÷^áÚ?ïøY0Pˆa?8÷-á?cÑ?N›?ÄC+?8÷-á?cÑ?ïúÃ"€r?G¥ÖV8_H?Dòxуæ?G¥ÖV8_H?ïñìä;Ì?­.™È¨ ?áÂe0Tˆ?­.™È¨ ?ïoå]½Jy?ŒÂ͓áe?'TO5èÝ?ŒÂ͓áe?ïmt†ûY?‡úÓ©¯M?'Qo6Ù*à?‡úÓ©¯MAGN3FGL J1215.9-1926@r8Œ?>q@ES3"l;'À:-H*;<íÀ;ºêßÝJÉÀaa;.T@—ÿÀ@Pwߊ"™¿éßv\›¿ãñ¨‹Üë¿Û€Sɱ¿í;=ž¤£ìUNASNone@Úþ§±PowerLawnone?ïj
¾R"?¡ø+l·±?Ÿr¾¤Æ€?¡ø+l·±?ïݽ8:?'§/aFé?q!9"²·
?'§/aFé?íÿ¸òÐA¡?œäLQY'W?°8k5Àó?œäLQY'W?ïÿúŽHz>ÌÀib»2ª>ÅÇï:>ÌÀib»2ª?îȍKO?¡V{f¤ ?£x'Ût?¡V{f¤ ?ïN—œáš?©D>²éÿ?–-bñI?©D>²éÿ?ìV\é"³?¯.™¢QC×?½M·†êj?¯.™¢QC×?ïþ¿§[ŠQ?.1ge¥|?$ŠÔÃ@?.1ge¥|AGN3FGL J1216.6-0557@qö8<òϖ@Kí@$³=°À:o®
ÅÀ;—\>Å7­?Í,Xæ˜ð@ü;û-Þ@Ý0ŸÚü:¿ç½žÁ¡ y¿ä°ÎøSÁÒ¿ãu7	àC¿ïýÌn®'UNASNone@ŠzF^‰"SPowerLawnone?ïðYå#±?`ϔ{@Há?_áL¶éíä?`ϔ{@Há?ïÌüÆ˽?…¾p'Ùø?yœ€´Zb?…¾p'Ùø?ï/‰Ð£Æï?‹
Â,د?šÅè†"?‹
Â,د?ï‡,ŸpH=?pÛaÚëë?Ž4Ø']ŒÚ?pÛaÚëë?ïïte"¾Ê?cšÜEØÕ®?`‹šCåÒ?cšÜEØÕ®?î4î8¾?´V7Í<Wv?¬¿þ$Œ?´V7Í<Wv?íÓ¥=¢ß?¤8.WœÃ?±gÔ[?¤8.WœÃ?êÒj=j?°˜ù7Ü1¼?ĶW÷ÒV?°˜ù7Ü1¼AGN3FGL J1220.0-2502@r_ÍÓØ@B¤!ÀD(NÀ:WfÛl7À;¬—AЄ迶
ˆnÚñV@ŠJ}Qº]@r`Æ%¿ïÆ»y$?ÜÎk6Ʉˆ¿è>)YÉ(¿ÒÈ*Ïj£UNASNone@œö#9ÀëîPowerLawnone?ïúO‹df?MÝ/R¡`)?FÃõùvÂÀ?MÝ/R¡`)?ïØÐàœ|<?ƒ8ÐÁü÷¦?s—'%zB?ƒ8ÐÁü÷¦?ï"Rt/ìq?ƒÇpá7?‹+bæFsì?ƒÇpá7?ïøBÆÆoÞ?;,ÏÕCß?NôäL-?;,ÏÕCß?ïÞ1lÅ·@?w@žQùjº?pçI••<	?w@žQùjº?ïÁóß>?­~P›ƒ×?œçÜf«';?­~P›ƒ×?î‹Ӟz? »Äź!?§NòËÃ^? »Äź!?ïá8®a?"»•–~°?Œ‡±Íˆ'?"»•–~°AGN3FGL J1220.1-3715@rAc@93MjOÀ:š¿3‡À;½ò×"'%¿ÎDn?´Üý@
ää~`y@_ßÿY'í?Þu`ZÄØÉ¿á· "IÖä¿â€BÌ=¿Í]ßØ\UNASNone@¢ù|í'hPowerLawnone?ïýçM›X$?,ã‹öÂrõ?0Ŕqï?,ã‹öÂrõ?ïÓüÇÄØÀ?"Ú¼ýág›?vœ; CÃ?"Ú¼ýág›?ïÚ9»sÅ0?l·Üx¯ö?rã"WKsú?l·Üx¯ö?ïúš'o'ø?2jOXõï?E•öµ¹"8?2jOXõï?ïúšY[R?D𡆱O?E–š¨HSÕ?D𡆱O?ïè»ü×?°ÀÓBS†?Ÿ¢è…Œ‡½?°ÀÓBS†?ïµëQû¨á?'/ÒZÊ3½?'…+y†£Ñ?'/ÒZÊ3½?﹅(¸Ú?x‰AÜëD?žµÕgå'?x‰AÜëDAGN3FGL J1220.3+6055@`4'¾‹Áj@Kå~ºñ6À:ņè¼í\À<  ‡Êd=?¼"Ze@9»n€'@#?¥‡d¿åùáéû˜¿éÙ¼06Bv¿ìv'"×?âK˜N­kUNASNone@t!ê5"PowerLawnone?ïxàÉ?¾–eOÕI?ãþ!"á?¾–eOÕI?ïá\Tjw?ƒKÑqm?n£«Þ('?ƒKÑqm?ï7Lâ´?™©ç‡ŸŒ?žy`Lm'?™©ç‡ŸŒ?ïÿ3WMø9?œ'?ø™?•èLÐW?œ'?ø™?ïØæ€Iˆ×?"a²ïÎPþ?sŒ¿¹hs?"a²ïÎPþ?ïCè¶üð›?§Z""y-'?—'é aì¦?§Z""y-'?í s3d—•?«ŒtçåUO?²üfcÿ\V?«ŒtçåUO?ïêa\*<-?oÁ0¸·È€?ež£¡‰Â×?oÁ0¸·È€AGN3FGL J1221.5-0632@ri$ò'Ð@KÆ YžØÀ9b+åaIÀ;'ÍDÁÐð?æöËA˜Œå@±VPÇ!@ÿ"_mλ¿Ý-V·$x¿ßìj…ôù¿áû`Þè]¿îÍ¡¸ÄN›UNASNone@"ŸË)^žPowerLawnone?ì‰c8Ù?»žêô!œÕ?»´ç¾?Á6?»žêô!œÕ?î¬hÿ¦qw?£;âsA?¥9p3•?£;âsA?ꌷý÷€ï?¬¥+ §0Ú?ÅÍ !üC?¬¥+ §0Ú?ëŽ!¢"el?š %Á-ý×?ÁÇywvjQ?š %Á-ý×?å4òNOU?Éhà¸©™?ՖùcaW?Éhà¸©™?æo®z7Ê?ËÄ!"´¹?Ó £àk?ËÄ!"´¹?å*}рÕl?¹]̱®j4?Õ«\þU'?¹]̱®j4?ÖÀ,G~I?³×ˆÄË{³?äŸéÜ@÷Ü?³×ˆÄË{³MIXED3FGL J1222.7+7952@_ Ò
ú/@B–-û¹À:Â3|.NÈÀ<%K#É¿è}ê!Ø~@ÅXlþ†?ûËÓÀ±ád?ïî·JÚnÌ¿Ü&¢¡U$Ë¿ßrøËXX‡¿¼ÖçzDŒUNASNone@½AO\(õÃPowerLawnone?ïÿù°8J?°$»ÞšÈ?À˹…€?°$»ÞšÈ?ïß]9|›?'I'`)7?pQ|sæ?'I'`)7?ïÖÖ©"Q?rÔF%l¹?t"«hç·?rÔF%l¹?ïÿ¸µÆ×>ô	Šù¸Û?ÒÅ»K!>ô	Šù¸Û?ïþVðQ·-?',¨Áuý?*ÿE 1?',¨Áuý?ï&i)þðÐ?¬ÉðÙ¯O?›2Ú¼²J?¬ÉðÙ¯O?ï¹k%èÇÕ?¼Z<û´?¥6ˆº·?¼Z<û´?ïüõßô$ˆ?7æŸ8I7S?8Q/Ãýœ?7æŸ8I7SAGN3FGL J1223.0-5622@r¯®]á\§@Š\å´$À9_7T*#ÀÀ;AiÂ;yS?è~Õp_c"@"üÄâ@4Ô@®¥¿ç£Äë¬â¿ç7Ì@\¿ìð³'ÎêοçG¾É1•WUNASNone@xhzáG®PowerLawnone	?ïáòxØÙË?wµ;ÈuŽ?n
‡Uàä\?wµ;ÈuŽ?ìÓg3üíã?·¯ªö¢Ùë?¹dÆ^ζj?·¯ªö¢Ùë?ï"Ô°	â?'¡jF»h[?œ;¥mn_³?'¡jF»h[?ëƒC}?›Ç‰¤!§?Àõòò±Ë?›Ç‰¤!§?îO4둀h?¨Eqy'¦?«±E0+"?¨Eqy'¦?ÓÂå˜Jº?ÐAV;Bn?æ3Ú¢ù?ÐAV;Bn?쌙£L?ª­Þïø?¿k›2åŸE?ª­Þïø?ÑÀù.æ¯?¶Ô·G—}¼?çühŒ©?¶Ô·G—}¼MIXED3FGL J1223.2+1215@qY ¥&•–@Rn•¿ðExÀ:Uÿ'E7BÀ;Ôzª3?âæêÖUÀ/@
^)Òâ:@´ƒàtÊW¿ë¸Kwn¿šº"|È¿ãÆÔ²–¸¿êjx"nëUNASNone@—Hœàu÷PowerLawnone?ï¦g$sÊ?"I[¡=?†f6Ü.@e?"I[¡=?ïW39''?—Ø%f.Æ?•˜Ê•#¹?—Ø%f.Æ?îœc i_ž?™šKþØ£ö?¦9Íõƒ+?™šKþØ£ö?íQ¥Øè?•êy1Åô?·…rØ%¾?•êy1Åô?î漫¨¡? Õh¡°è‹?¡"5Euïµ? Õh¡°è‹?è½Ç‹;Õ;?ÊÆñ>yÀê?ÍáÓ«?ÊÆñ>yÀê?ìîÅM°?¬gÒêK¢f?¿X‰Õ'Z?¬gÒêK¢f?ڜ ³ö?¸¿0Zzo¿?â±ï¦8÷?¸¿0Zzo¿MIXED3FGL J1223.3+0818@q¢éxÔýô@Q'êžnëpÀ::H=†sLÀ;ËÿwD?áP½R¡Û@
÷Ú·R?ÿÁìžú+«¿å6l³)(¿Ä¨M ‹•¿Îy¨çH¿ë÷4£[ö\UNASNone@£/ÓÃa@PowerLawnone?ïd	ôdZ6?'Û€ÜÃÁµ?"~Áu,‡/?'Û€ÜÃÁµ?ï–d~bd,?'åKûz?Šfàu%d÷?'åKûz?ìäýΪü?¨*ô(§?¿ØŠ¨ ?¨*ô(§?î?F‹nwq?Â†Æ&™?¬—F"Óø?Â†Æ&™?î_èÉ`9Y?ªInŒdL½?ªsjØQj?ªInŒdL½?잘Ã&?ÁVê©?¿Ã9çNÑ?ÁVê©?ìtÈKU5?¬Sb€7NÊ?¿4Y½¥VU?¬Sb€7NÊ?åíŒô"YÐ?À!ž?NR?Ô$æ»La?À!ž?NRAGN3FGL J1225.4-3448@rŽg ù	l@;†ƒ<`À:ºèÊYUÀ;á'o°'¿ô±ó:ß¿@1PÊÈ»›?ü'ºž÷Ò_¿Ö25ÿ¶¯¿É3Yö¸Ðä¿ß­[ÿkl?»}ÙI²ÑyUNASNone@»H5$ÝPowerLawnone?ïýt´K»Y?2' ™¶Á´?4Z\wf?2' ™¶Á´?ïÛZ¶͊?'¸¼",\©?rR¤ùXJâ?'¸¼",\©?ïÍÁè©]m?u¤¸ç²=?yľeH?u¤¸ç²=?ïÿñ
ñä>Õ`$|d>ÝëPC
˜¬>Õ`$|d?ïøÂê©_=?J–øXë?LôU*"%É?J–øXë?ï0¿QhŒ?®ZÛÝz³¿?™èá:Xq?®ZÛÝz³¿?濾Ù_¥?…bVQêZ?†^þ‡NÎ?…bVQêZ?ïþ´+ýE!?(Iëç&…í?$½@ :K~?(Iëç&…íAGN3FGL J1228.4-0317@r;jžnëp@M‰‹ÖbwÄÀ:ìÝäLEÀ;¯
õ´MÀ£$u«'á@‹ÝËø'@,û GH>¿Ìˆ©'
.,¿á™âGeù¿ßX#¦ô¿åôŽï`d^UNASNone@–ˇ"Ý—öPowerLawnone?ïýlȈÍø?A7–èöpë?4™»@žã?A7–èöpë?ïàKd'`˜?´Î2cc¬?o´›x ?´Î2cc¬?ï´î€•€t?'ýL5"?'Ä_Ò¸É?'ýL5"?ð=Ô\§[™
Þ=±¤¬R†7=Ô\§U$6Õ?ïùrA]d×?PH«‡	¤?J6úQ̬J?PH«‡	¤?ï^9µó_?§Û\Vžñh?"8É:À?§Û\Vžñh?ï7ßFeÙ½?–…y?™3DÈS?–…y?ïÿÿýÚ>ƒ>M|šX"lK>/'k>M|šX"lKAGN3FGL J1231.6+4825@`{ԕ*™@Q`þG™À:Ø£š¤À;»‡Ý¯s ¿º'÷‡
¡@WÀ<pž¤@À‰G'¿å&ËEä¿åV c€`–¿ëQšfÜó¿ÛGÎûü[UNASNone@ŒœqýÞ½PowerLawnone?ïþ•S'´?1Xèã	0?&ªË®'ˆ
?1Xèã	0?ïâ+°G?'1&C>?mÿԋS?'1&C>?ï·+Ý Ñê?xåсÚ?'5¦é͇?xåсÚ?ïíq!wÁO?O¯~ Ÿ?bŽÞX$)6?O¯~ Ÿ?ïö¼xÊJ?X`¬áœÄ?SچÌrìÕ?X`¬áœÄ?ï"µ2ëÿ\?¨%®ÇE}?›©Y¢€…?¨%®ÇE}?î×cå,À?œºŒQ?¢Ž¹¿õf?œºŒQ?îJ¬–Ì_À?£JÆ×þÍ?«U6•Í¹?£JÆ×þÍAGN3FGL J1231.7-6513@rÍ×süPÀqOøÃÌÀ8Ác¡ À:ôóW{?óñKle@üóʒŠÝ@e#?ö;¿àÐ9zŽÖ6¿å¥+XÚs¿èd1®ßã¿î‹ºù¥)UNASNone@‰Ö}!ÿ.IPowerLawnone?Á›ä0°eÓ?¾O»K'qÿ?ë™óÓæ‹?¾O»K'qÿ?ÄæÔ|r?Ãorðs¬0?êÆJø ãz?Ãorðs¬0?æ«kTтX?°wYD!?Ò©)V\ûP?°wYD!?Û°bæK›V?¦[' NT!?â'ΌÚ2U?¦[' NT!?'oØß3?‡|šÅoŠ?ï¶C"Ù?‡|šÅoŠ?˜xøH\æ?°c}sù@?ï<8;ÊuH?°c}sù@?ÐÙ	AÙOx?µÄ>ú4ç?ç"{_XD?µÄ>ú4ç?®0ýñ‡í?'Mñs¢?î÷à ç?'Mñs¢MIXED3FGL J1232.3+1701@qeŒûüeA@S¾7`¿]yÀ:K1"·ºíÀ;·­AJÅ?µR"Ž49,@
» ì^¸r?ýeÀÂ}i?â÷ñó;»1¿Â½¾ßE¤¿Þ}4B@±¿Û¹'¿ÚÃRUNASNone@«"t¼PowerLawnone?ïþWéöÔ2?&éúØNøÖ?*d7£R?&éúØNøÖ?ïÝÝŒÊ?‡´ Âd?q{˜ž½0?‡´ Âd?ïÚ՞$K?kž#—QD?r•0ø÷O?kž#—QD?ïãk"æ–?T/ÂtàûÏ?l"kÜðÏí?T/ÂtàûÏ?ïú´§&n?C¨ˆØ8Á?E-dw÷=i?C¨ˆØ8Á?ï/?LA!?§HRnÖ°"?š]WÐ?§HRnÖ°"?ïº?ڔP?—ÿ6Oh?p	YC]æ?—ÿ6Oh?îéçë"Á¡?"TÐø="?¡aE×þï?"TÐø="AGN3FGL J1232.5-3720@r¬r䎊r@9`œä§´åÀ:Eä9ÐÜÀ;Ã3{W3¿ËÝ«Pj‹@#
%­c¦?þ˝_¡Ñ!¿ì¾WýJ¡—¿ÍpºZâØ0¿Ù2҇™3e¿Ô"•ziíHUNASNone@®Àœ"µÜÆPowerLawnone?ïþÀþk? ¯òÙ¢¦?#ð/òH? ¯òÙ¢¦?ï՜oüc?"˜¶@çs?u1È~ÑB±?"˜¶@çs?ïçäþƒ?jAq%8t?hâ
ۉv?jAq%8t?ïýóiܕ?z²á,Ã?0d±ð=Þ­?z²á,Ã?ïýҚ'oA?/Œãœdd<?1k-7[%?/Œãœdd<?ï¾Kw3?°zî8?ž(6Š=¡š?°zî8?ïâJÕ]·c?tÂm+C9?mµ*×â…?tÂm+C9?ïî@/¬&?VVM«5Λ?aíÀ.o?VVM«5ΛAGN3FGL J1232.8+1332@qÅ)ûçl‹@RîÐ=š•BÀ9þ©1½nÀ;'ÆÞOâ?֕YscÏÞ@o÷oF@]o€–hb¿ç{YŶy¿äœo
éÓ¿é{€cŠ
}¿ïþ2£nQUNASNone@ƒÅ"¿	•«PowerLawnone?ïÔ9£µ§?uŒ×S`g°?uãt"v€p?uŒ×S`g°?ï¿ØÜÜ\?‹ªX"ÒƝ?€	øJ(Á?‹ªX"ÒƝ?î¼6÷…T‹?"–40õpy?¤<‡ª·W?"–40õpy?îÁÀtF?"ÄÀœX¨?£îg°‰™?"ÄÀœX¨?ïäaòkö?Œ¥€0%²x?Œçy.z?Œ¥€0%²x?ìyU{Ú?Ã/w/L?¼3…W\!-?Ã/w/L?ì´üå!
?¨[áV)?ºXÖ÷¯5?¨[áV)?âÁévü‹¬?ºa•­b	œ?Ú|-è§?ºa•­b	œAGN3FGL J1234.7-0437@rqe"¯O@LÿŠC»@³À:ŠE{4SÅÀ;³"¢Ù´?Ùôÿ­@êI5Ó÷c?úb¿?›vi¿ïÕ@–?"b?åÝÝ*_qw¿ìõêÚBÅç?è\k˜ÕN|UNASNone@ÁHñ©ûçPowerLawnone?ïõv§Q=4?\ŒÑ=A?U±Öwֆ?\ŒÑ=A?ïÙ繦ï?…ÞÍ6qZ?s#4nj¹?…ÞÍ6qZ?ïb™×?‹ŸÙä2P'?"¬ß¡¯ i?‹ŸÙä2P'?ïþ'_wE?.G'O\Ã?-‡æz&f±?.G'O\Ã?ï™èZœÚ?1ƒyªb€?‰»ÅìÈe–?1ƒyªb€?梨pÙ?®ŠÇ†Ì>[?œ«Ò¬ô?®ŠÇ†Ì>[?î"FN¡M?›°KaÓ.¼?¦Ë›Ÿ¹+?›°KaÓ.¼?ïÏÀÙ¾;©?"ìŠhŠi6?x"6ß«C?"ìŠhŠi6AGN3FGL J1236.5-6154@rÒЛùÆ*?íSó.ZÀ93»ËóˆùÀ:Ÿlç‰çu?ȐÝ,Y›@Ø+Ú#w@ð¸`Y1¿è­ˆÖËÆ¿ã-\òÓô¿é½)Æo\ü¿áI踪oÄUNASNone@š¶œ¬1'PowerLawnone?îÉ·5$¾À?­³L<&ss?£dŒ©h'?­³L<&ss?ïajÉÖ?­ߟ+aª?"Ò¦À•j?­ߟ+aª?ì}ÅB¡?«Á‹zAñ"?¼×÷Uê÷?«Á‹zAñ"?ïåb*
?Qënä¿PÆ?jåö¤?Qënä¿PÆ?èlðñÅ)À?Șã'4pJ?ÎL<8ëXÿ?Șã'4pJ?ë_d©oG?Æï÷¸øs?'mZBãø?Æï÷¸øs?ç'ZQžó?º´›Šðþ?ÑØûK\Â?º´›Šðþ?î«ÂfŸúº?•b'"
Á?¥CٚK×U?•b'"
ÁAGN3FGL J1236.6-7050@rÛMžƒä&À *™0¾À9Ôÿ¢³õÀ;dÎ#"¿îÎ2c»¢i@ß	»?²@©c `Ș?íM³ØØ¿ä##À›Þe¿ærQ2;€N¿ÝÒ"…¶¹UNASNone@Ÿ‰èr° ÅPowerLawnone?ïøµ.~ ?`;3´lÁ?Oå*Õá@?`;3´lÁ?﫬£6¦?'ÁF]'¾t?…?ÔÞŽ`?'ÁF]'¾t?%TÅ¢?'@Ü2¤ó?‹v®>3›?'@Ü2¤ó?ïÿfƒ}ߐ?­iywÈ?/‰Ä¶§8?­iywÈ?ïîéz¶A?cæ#–KF&?a…qÔ6®?cæ#–KF&?ín2•©u?ÀaWšÇ?´ŽkQØpâ?ÀaWšÇ?îÏ8;S?™Œ=¯pÂ÷?£ÿºké?™Œ=¯pÂ÷?ïöþò1?O
Üï(?Rú7H~?O
Üï(AGN3FGL J1239.1-1158@r£6âë@IdÿñÀ9­Öû#ø-À;"ÙHÜ?ñ10N§X@D£JÈP;@ˆ ÀaŠ¿êä¿hìt¿ëäQZ)…ú¿ÞÇ\O≿å'UZPUNASNone@p⇓ݗöPowerLawnone?ïóþW¼Ýõ?Zúb$–ñ÷?XPbˆ&P?Zúb$–ñ÷?ì°d	Ðõb?ºT9¤L·?º|ß±xTó?ºT9¤L·?ï1W²)Ć?'öõàÚZ[?™Õ	·WÓM?'öõàÚZ[?ëøÍ(3È&? Aû& ?ÀË_0ßh? Aû& ?ïíB¬´Ì?iü‰)c,?b½S_/Þ?iü‰)c,?ß´žšÍ?Ñ-hjÄçH?à%°¸2ûš?Ñ-hjÄçH?í¡Ü+9"¡?¤LYÛú£[?²ñ¤{Œù?¤LYÛú£[?ß2$'( ?¾zAm;J?àfí¶ëþ°?¾zAm;JMIXED3FGL J1240.3-7149@ràÝDUGÀ!ò7Š°ÈŠÀ9NÅÚjDAÀ;PPKqîZ¿ô4ÏÅЄ<@ÿ÷1Ð1±?ÿo¤?åÉ¿ç3àÃ¥v¿ãü!‡ Y
¿ÛyVÿ§PοÒíƒ~Ø«±UNASNone@¬±<64PowerLawnone?ïüîó4·å?3tIë·þ?8ˆeg™Ô?3tIë·þ?ï±êê€M)?'Æ~a×KÜ?ƒ…EkóWÌ?'Æ~a×KÜ?ïêº]o®?f•oÅ3"?eëEÆLAÚ?f•oÅ3"?ïÿó«Ï§>ÑH7.«>Ø奊ø)>ÑH7.«?ïüǕ¯?7!I
è?9ÃXò ?7!I
è?í¾ìù¬Ã‡?¼ô5OÖh?²˜3ã¾H?¼ô5OÖh?ï̲~͙?Š<Xo³?y¦ýJèp?Š<Xo³?ïÿhì[;?ZÊÄRÒ?ârúQC»?ZÊÄRÒAGN3FGL J1244.2-6227@rá˜ÜÛ7Ê?ÚbÅGtÀ8¹+0/sÀ:~"Ž½ž?ñZ:MƒÁ@
°(ù°@—kˆ±j?ïþßZ)Rp¿ã6âƒ~‹\¿ædæo=Ù¿ì¬wJlé@UNASNone@™;çl‹DPowerLawnone?£ûàØ͸?®«#N¡"3?îÀAòqTµ?®«#N¡"3?ÔàV­òÓ-?ÊSèEµ?åÔ©–j?ÊSèEµ?ׅ_%ºF?´ŽÝzóOé?ä=P9m"Ý?´ŽÝzóOé?âÏ(O]	?°­Z«°
?Úa¯aEÙî?°­Z«°
?x_ÑGk?‡Nd¾¥Ö?ïÏÙ@<tê?‡Nd¾¥Ö?­£äº?Ë?²ùµù°w?î%ÁµíbD?²ùµù°w?³¹lc{ ?¦©ÒXÊ=ô?íˆÒœËÜ?¦©ÒXÊ=ô?ÃÑÕ]"?§àr	's?늨˜˜›?§àr	'sMIXED3FGL J1244.3-5515@rޗö+jè@gB™ØƒºÀ9_ýŠÚ¹õÀ;O¦¢–˜]¿µ\)^ŽÄ@«wÈ8"o@õò`L–¿âX´^ìÊn¿çt|')ð¿êŠ'=:%É¿âE&M¼ŸUNASNone@€¼<j~ùÛPowerLawnone?ïô`')!{?[´Ù'°Yã?W>Ý°|¹?[´Ù'°Yã?ïª,#ýé®?'í¹$¦?…töïWˆŸ?'í¹$¦?ï'Ѹ]ÃÄ?ƒpEjö̃?K'ëþªæ?ƒpEjö̃?ïÝ ûÉË¢?XGßùŠ?q/'kƒ3?XGßùŠ?ïuÎqEE7?•-n¼åèÁ?'F1Þ6'?•-n¼åèÁ?íl£Ž²W?¾|Oq¨?·dšád«É?¾|Oq¨?íç¸î@x?¤KÝD¶¨?°Â8#åD?¤KÝD¶¨?ís–Kl¡$?¤uŠìc³1?´cM¤šöÞ?¤uŠìc³1AGN3FGL J1249.1-2808@rå2a|Ú@A\ÚãæÄÆÀ9Ý68¡1>À;ªíñ	Â÷¿ç•ÿø€§@E
6ÊA'@ˆ‹`pÙ¿èÛÃoMb+¿ß)ŸÑ`I¿Ýj…ÿLÀ'¿ÞŽk›¸
UNASNone@¡u	^ž	PowerLawnone?ïþ{"ý«ð? +	r Ȁ?(FÀu,Ñ? +	r Ȁ?ïÚeaXµy?ƒ!µ)"‡g?rÍObŸˆ?ƒ!µ)"‡g?ïí"ì'þC?PÁ¯×+r
?blµ¥¤ü?PÁ¯×+r
?ïþ¨&¥0Q?å‰Ó6Ú?%}"lÖ?å‰Ó6Ú?ïüí0µª?3Û?xI¯?8—¦'ƒ‡?3Û?xI¯?ï26üìO?¬,2Úe@?™¼ƒ> ?¬,2Úe@?ïêgŽçT?jí›ÿÑ?e˜qæù$?jí›ÿÑ?ïëC wU?^P¢Cí›?d¼ß¨G`€?^P¢Cí›AGN3FGL J1249.5-0546@ràë…¸R@L‹fÉûÀ9óÔCédÀ;mQ¿tè¿àAg©\…<@³g€Â³@M¤`r¬?ïEcòmÆ,¿íc\›·¿ÀÁÁ‰¿è¥åÊʔ
UNASNone@–µ&Á½¥PowerLawnone?ïû_cà«?E¼FŠX?B'o†‡=
?E¼FŠX?ïÙìL™â?ˆ{
§?sy‰Ý"«2?ˆ{
§?ï¡Ç¹|?ƒ®" ÈÄ?‡¹Î  ð?ƒ®" ÈÄ?ïü»ujÿ?*cm"V;W?:$TÀמ»?*cm"V;W?ïý6´Çó?<`lÒ&?3–J¬7D?<`lÒ&?ï6ý>üâ?ªø>ÔFÖ¹?™= T°Ç¹?ªø>ÔFÖ¹?ïVe*¸K?º"&¾üB?•3Z¥†ðq?º"&¾üB?ïíÞÌòó?\/îË?b!3îM\Ë?\/îËAGN3FGL J1250.2-0233@rå'¡ Ï@N'=¯÷¥À:—öÅĚÏÀ;‰Øê2¿Ô!‹ôs
@
5I¯?ñ€y¿ïôÍÁᮩ¿á Í‰¤ó¯?ç³p;Á?êX•íUNASNone@à/œPowerLawnone?ïûlkýÃÔ?P0™ñrˆ?BNO8od?P0™ñrˆ?ïܸm]õ?'Lfj­ì?q£É'•W?'Lfj­ì?îrýÓÕՊ?¢6¨ \Q?¨Ð"Àòc?¢6¨ \Q?ïÿõ¾*>Ѐk>>ԄàÇ2'>Ѐk>?ïûŠ³õ¢?DðQïï÷¼?A×õúxß?DðQïï÷¼?ï;"MæEw?ªp›ˆ,ù?˜›¶J‰
?ªp›ˆ,ù?ï•ý |¢?Œ9>c]µw?Š¸şG^?Œ9>c]µw?ïÿä†ýµ£>ô*Lê'I>ëy(N\k½>ô*Lê'IAGN3FGL J1251.0-4943@rîƒùd@*GЍK­}À9ÖBƒ2OÀ;tˆhî?á;­2Ü(é@¹ÈQ½âÏ@=ÍØã\?æ7€y%õw¿Õó(¼6Òz¿ÒÖ"¿{30¿é¡¿+é+ÂUNASNone@¥«»=ÈKPowerLawnone?ïqÏ£õEÅ?"é>ïë:?'ƁWGS?"é>ïë:?îØ|Bh&Ò?¤!†Iš?¢x;Üí.×?¤!†Iš?î¯	1Eáû?œB¨¦{?¥lî5•H?œB¨¦{?íـ¥èî}?î]Š,Ã?±3úєs?î]Š,Ã?ì}ø4â?º1A&Í?¼ø?þXò?º1A&Í?èŒþâãSf?Éf¬]æC?ÍÌtr²i?Éf¬]æC?ì C䨮?®®žíÏ"~?¿žýàÚº?®®žíÏ"~?åùŽ	K5ç?¶.Z7âx?Ôãíi"2?¶.Z7âxAGN3FGL J1256.1-5703@rùHè§ç@Bæê…DxÀ97¯h¸À;Ð߁w?òùéá½)@weêÀ}´@Š<€c舿æ"ŒéC)¿è-¶G¶^2¿ëûGC,òÊ¿ì/%\…èUNASNone@€é´¢3œPowerLawnone?çŸN"¸‰I?ė#"ú?ÐÁb֎ín?ė#"ú?Ý?òó–ÔÝ?Ê,)/4‡,?á`†4•'?Ê,)/4‡,?ë‡]…*?¨ð^p=?Á⋃‰ëY?¨ð^p=?äEúi×ÎÍ?¨›‡ÿj
M?×t,Pbe?¨›‡ÿj
M?Ü»¬–˜Ö?Ëôðh™ƒ?á¢s©´³•?Ëôðh™ƒ?³ÇrY¡²?¾ÿU(Y(?퇴³Pz?¾ÿU(Y(?áŒQZn>*?»Ùp°R~ä?Üç]K#ƒ­?»Ùp°R~ä?¾ðLJ?¤1ãwÀ??ì>!ölO×?¤1ãwÀ?MIXED3FGL J1257.0-6338@røт©"¿è¨À~	ñÀ85«³w'À:‡/	ØÆÖ¿¤8Î@ˆr@ÿqŒ_Ig@ò]Àz"¿ìÞ—ÈšI¿ÂBfÊíØ¿âGŗé¿éY˜ÖëUNASNone@ ƒrþÅm]PowerLawnone?ï¾!Ÿ%l?ŠÀÅK†ã ?€wºO‹?ŠÀÅK†ã ?ïr՘€óc?©6à{{-?'¥LöÀ˔?©6à{{-?ís8©¿¬~?¤½ìZíȁ?´f:°¸Á"?¤½ìZíȁ?ïûm
^A™?.y¶ÏI?BK×pŸf?.y¶ÏI?ïD P<%?›ý‰ÄišÜ?—kíõø{c?›ý‰ÄišÜ?ì^"NØÅ?ÅS8Ä.¹?½ïå‰9Ù?ÅS8Ä.¹?ì~ÓӄÕp?©EšûÚ±†?¼	acÙT?©EšûÚ±†?ïå[ÄÕ?`	X§e?jæè¯9êŒ?`	X§eAGN3FGL J1258.4+2123@sî˒:*@Ur\=îxÀ:1—¿¤ÆÀ;'UÙPhÎ?ñ[Õcõ@%ÅäêÑ@&K_yã¿ë¾Î×û¿ïÿÕÝÚ?ïýåu²¿ä§B"èe7UNASNone@‰sÐ|"µÝPowerLawnone?ïó''$ç?_ŒŸCPYƒ?Xûò·:'é?_ŒŸCPYƒ?îåm_˜±?²ë[N_}w?¡§	'r¿ù?²ë[N_}w?ïIŽÐy?'Ô#&wm]?6Î.‡ãö?'Ô#&wm]?ïOP£í–­?"·/Xgˆ?–ëŠä0R?"·/Xgˆ?ïóÆæ®Ë?d¾8‰°)À?YÔr[ݹi?d¾8‰°)À?ë "š?ö?ÈÑüÆ,?Áµ±—&?ÈÑüÆ,?î9ÍO˜]? 
ö–.\?¬nS)N¬+? 
ö–.\?îәöi[í?²]Wb2z?¢Æ`šF(3?²]Wb2zAGN3FGL J1259.3-8151@ró¦">jÀ2þRv‰ÊÀ9Ê=|bQ.À;€ü‡7?âã"˜A'@Aà;i@'æÚ¿æäNò_1¿ã-=À!e"¿åSÐÄþø¿ìÁsnUNASNone@ñþ($xPowerLawnone?îÆ.Þé}?§yûê?£}³6?§yûê?ïU²ÜX(? ~KÔLšy?žI¤tû? ~KÔLšy?îXM,TP?˜û^^ß×?ª{-;Û?˜û^^ß×?í¶½‡Æ™"?‹AÄ¡–é?²JÁ]?è?‹AÄ¡–é?啉bˆU?ÍõMxȂ?ÔÔí;ÆïW?ÍõMxȂ?ã2Ôå0W?Ïì+	̐?ٚV5ŸQÈ?Ïì+	̐?éÒº£¤?³%%ÂF?ȵq½mÅ?³%%ÂF?àP¤HQÛó?²î%Ö?ß^·o\H?²î%ÖAGN3FGL J1259.5-3231@s™" ä@>Rb˧2ßÀ9Œ‰B37À;p—"6À
eS®þ° @{X³|@¶™ßåƒR¿éÎ]àÓ6k¿çO¶UU᣿çZaµ?¿ïÿ	̀žBUNASNone@{™¤?åÉPowerLawnone?ïÞp©Þ?q€»72K?pǹ4cÖ?q€»72K?ï܁é#ł?'²Y΅?q¿†ÚnÞ?'²Y΅?ïJºJ¶~ú?ŠX^±~L=?–¨¶¬Ÿ¼¼?ŠX^±~L=?ïÿÿLh0>™ ê'4É>¶.bˆ˜Õ>™ ê'4É?ïÑuÝ
?~&cÞj?wE{Ae?~&cÞj?ïCMšñ?«Ò½Ùh1Z?—Ÿ–Sñ?«Ò½Ùh1Z?î Èû"?"¹µî?¥ópS
éÚ?"¹µî?ïÿ۞]	>ýÌÎøùº>ò0ύ(yM>ýÌÎøùºAGN3FGL J1301.5+3333@Z1ûµsë@TÍ+©ÑöÀ9þêUrùÀ;Ö5À¬-?ïôÐp‡õ@'áÂ@-g߸6é¿ØT˜Ñl‰¿áLçee›¡¿è³vH q"¿ïÿÄoAgUNASNone@`ùrGEPowerLawnone?ï‹8]>Ÿx?˜U:cÙ?1è³Ç½û?˜U:cÙ?í!¼¶²·«?½ŸÙ±"m?¶òJjB¥?½ŸÙ±"m?í<°…¡óŽ?¢ª}"ÑB?¶{Òðc'?¢ª}"ÑB?éÉ/PÖ?¢çK¾šZ	?ÈÛC®¼§¢?¢çK¾šZ	?í[«óŸ†?¸›¨ö˜s
?µ'¢ˆÅP?¸›¨ö˜s
?å"]Dv?ÑñéR`í?Õ»EwÃè?ÑñéR`í?æTN
úÛ?¼0=½{?ÒýWcê
J?¼0=½{?Ño{-GáÁ?²#Åses?çHBi\ ?²#ÅsesMIXED3FGL J1304.6+1200@s³ …±…@R£öÓ0"À:¬Š7&À;¾òâ
K³?ê$.Eì&@µ[©Éèl@ü[€YV³¿Ö¹®(8Ñ¿â*5è3¿î;²[ü@¿ìÂ[¹ì1UNASNone@ŽX'RT`ªPowerLawnone?êEA@ù*µ?Ã^Ãwìÿ%?ÆêúüU,?Ã^Ãwìÿ%?î½±ÑɶÃ?¥çɋüWg?¤$â∬Õ?¥çɋüWg?ìl5NQ­Ù?¤Ñ…)†G?¼žUr'9?¤Ñ…)†G?ëOñÃ.ñä?ŸÚƒÐ¡Æù?ÂÀ8óD8r?ŸÚƒÐ¡Æù?år˜P™J"?Ë¢-7¬Ð¿?ÕÏ^Íj×?Ë¢-7¬Ð¿?äÛL%Õ?ÐF¬FðTf?ÖIgµúUû?ÐF¬FðTf?çRÈ-ù?·­æ Pš‡?Ñ[øo¤
ø?·­æ Pš‡?Îk72¾–?´o†t[™?èe23P[Ú?´o†t[™MIXED3FGL J1306.8-4031@s!° ě¦@6>]ž@ÈGÀ8ñjwmçÀ;ëÃ2X¿ò]kÑ@;®õKq@SL`UÖ ¿æ¤2
$'R¿åðÎ5úÛ¿æ2ÓD
Eÿ¿íHˆ,[UNASNone@‹¬¥zxlPowerLawnone?í³:މsî?³¤,ᢁ?²f)
Øy"?³¤,ᢁ?ïÒہgëï?‡¸½ï?v'?`§°j?‡¸½ï?ìœu[?¥Bùo…-ƒ?»ŒU'>?¥Bùo…-ƒ?ïøÕd~W?C²Lê?'?Lªn,Òÿp?C²Lê?'?êqsë_4?Ä^ÜX†?Æ:0Rƒ/ ?Ä^ÜX†?îöëîr
?°‰*ù]‹? 'A $Æ[?°‰*ù]‹?é¯nCÄ>Î?³Bš.ü?ÉBFðïÊ?³Bš.ü?îû~øޕ?›<rd0-? H€yä¨?›<rd0-AGN3FGL J1308.7-5738@s4Á¨¬\@jOvÀ9`Ö@†À;"ŠfðÀ^õѨԠ@+[Àðöx@mª_åmØ¿é¡XØçÀÍ¿êöbªÅ¿ãN`5IãÏ¿å'ärʑ£UNASNone@ƒ‡!-w2PowerLawnone	?ïáÎb_Vä?‰ g§Ïª\?n1Ç$»ý?‰ g§Ïª\?︉Á+Ñ7?û0LñË?Ý¶kŠ[?û0LñË?îâ¥'R'?›j¸췊?¡Õ­ŒŽÅà?›j¸췊?ïÿฒL>ð#‰LÈ·>ïGjû*ÌX>ð#‰LÈ·?ïÙøBW¤"?}ÇöoVÿ?sÞ¸°Öº?}ÇöoVÿ?î?@sHÞ&?¹'GáÆ"?¬øÌN—?¹'GáÆ"?íjš<W?ª&%ñ­`?´¯{äBÌ?ª&%ñ­`?ïû1¨ÞIç?EC¼¹?C9]'ì{(?EC¼¹AGN3FGL J1309.0+0347@sžoü]ö@P'`A‰7LÀ:—10#´:À;ð3PD¼?ðÄð_y@íyj¥@¯i\e¿ãS÷‡û%j¿¹U&œ"À1¿ÑÒÛ
8yT¿ïû|Ë`DUNASNone@žÓ=ÈK^PowerLawnone?è‰pQKÍ?Å'Ä	Ò?ÍÚ>ºÐËà?Å'Ä	Ò?銔Y¤ó%?ÄA3±³@à?ÉÕ®™l3k?ÄA3±³@à?é|ñ-æSm?®àÉÖc©'?Ê;Hf²M?®àÉÖc©'?è™.xb?­ÙpÃ8XÊ?͛G¾wÿ?­ÙpÃ8XÊ?çGöhá?È?‡'¹‰,?Ñp/Ôü>?È?‡'¹‰,?ÛíQ…6hÐ?ÐNL­ò[?â	W=d˘?ÐNL­ò[?äX`hÂÙ{?¹ÝR«ôe?×O?.zM	?¹ÝR«ôe?ÖƩ΁>?Â4'ôT"ò?䜫¿`ö?Â4'ôT"òMIXED3FGL J1311.8-6230@sœàuöý?ÑW«ãs,rÀ83¸"0¤À:,[Ðá."¿Ð GÑ®g@©h­¾i³@ªÚÀ«VZ¿ãH4qC0¤¿èðݯte¿ä=`
¬¬¿çõȝNk.UNASNone@'Ö}ó¶E¢PowerLawnone?äÌãí?ÑîGJ8Ö?×âüf9è&?ÑîGJ8Ö?ïf"Ryc]?¬±6¥JÖ'?"/u­cøc?¬±6¥JÖ'?ãÎ}–Ù Æ?¹âIá nu?ØcÒL¾u?¹âIá nu?ïÞSͲzç?a_>×{ì?pÖ	åÔª?a_>×{ì?Ùýó[³§?ÐÑ6æ"iÌ?ãtR&,?ÐÑ6æ"iÌ?ë—ÚûõÀr?Å1OG)Îõ?Á "(þ7?Å1OG)Îõ?ãM±+[£j?¸Ëó®«'?Ùd©H¹,?¸Ëó®«'?î9ö³ûð|?™1¹Kë¯Ê?¬`"À@øC?™1¹Kë¯ÊMIXED3FGL J1312.3+8513@^šâ:¸c@?á鞔«À:5-ø`ÏNÀ;ޓ*êU?Ó-}*'èº@
ì¯úÙû_@Œrk­¿èRÔÚs«¿æPÒLàѿ旤ØÿпÑÚÍì\ŠUNASNone@†ÔoiPowerLawnone?ïõËÜÚ-? .(®á.£?TàgþÓÅc? .(®á.£?ïËiX‰?…•Àlë?zKqfI^?…•Àlë?ïn°Mvf ?½?W¹?')öRêú?½?W¹?ïm,ds-?v(¦]f~_?Œ¤´ø@'?v(¦]f~_?ïõF0Äv›?`ØBÆÈ?Usž°Ì:}?`ØBÆÈ?층ʉ?¿X>3ÜW?º<WÑ«·?¿X>3ÜW?î'frƒ]Ì?Ÿ–OWïÈ?¦é˜Ø¦
E?Ÿ–OWïÈ?éJIæ?½HÏQ·WÆ?˞×ϒØh?½HÏQ·WÆAGN3FGL J1315.7-0732@s—+Iº@Ki¡lçŠÀ9f'áÇ/ÕÀ;'N+Üýœ¿ú0qÅ?9Ò@"étù&@'JßÍ/ž¿Ìß³={¿ß,Lâx8¿åœVK·u¿Æ·ŽgUNASNone@ g]cˆfPowerLawnone?ïûPeÉ›?A"ÕÚ2?B¾hþ"ã?A"ÕÚ2?ïÝré‡C?'<'EP
ì?qF÷£ùŽ‰?'<'EP
ì?ï®å@??€é¨'äd?"{¿?иZ?€é¨'äd?ïÿûmŸÙ>½
(¥Ã>ÂI—g®ÝÐ>½
(¥Ã?ïö'ƒ''@?QÛÔÄiY<?RúùâUßS?QÛÔÄiY<?ïJ.ÔÌ?©§Çð¼c?–º%_åÓ?©§Çð¼c?ïW{‡¤"?·6¬r5é?•0m"?·6¬r5é?ïÿ‡‡¯?ÝM#¥pÅ?>M°:…?ÝM#¥pÅAGN3FGL J1316.2-6446@s/D')‰À3¼$ÞܚÀ8{¾öJt˜À:Åe˜Tö?à;'1ÈúÛ@¨/t··è@O"/û›¿èeà
éš¿èd€k'ôÄ¿ìÈ`´u½ò¿áÝüó¹©7UNASNone@wòC¿rq7PowerLawnone?ïþ6¹qó…?41‰²ƒªC?,"iÁ™A?41‰²ƒªC?ïpT:⠓?¡âÚ>ö?'õxª›%‰?¡âÚ>ö?ï
1ù;{?•êãŸ]d?žYÀڈôœ?•êãŸ]d?ïâ·Gpy?RYà¿È€V?mH¸Œîa?RYà¿È€V?ïàBéð°=?t\«fEJ?o½7+:Ã?t\«fEJ?ëƒMø[pê?ƯËpg'V?ÁòÈ'<X?ƯËpg'V?í1ÒÇò?¨¤v"Zä?·Žqhë)n?¨¤v"Zä?îì¼ó!0?'ïe¶º¨?¡40Ì5)+?'ïe¶º¨AGN3FGL J1323.2-3901@sZ‡ÝDU@7nhãï(AÀ9ËøÁG^À;q½OH¿ÙõÜûîùG@ŒÖ脎@.Yßð@¿ãÍZÐc–¿èœ±ûÔææ¿ã`C˜õɊ¿éh=2v±UNASNone@‹–¼j~ùÛPowerLawnone?ïôågáö?VÛûäžlë?V52)±sè?VÛûäžlë?ïÍv›ÆM4?‡¹¤2+$?yD²šUÔ?‡¹¤2+$?ï'duÃü?"OÀågh9?‹fûÔА÷?"OÀågh9?ïáK¼´ë?WˆÈ¦K}ˆ?n´íCK?WˆÈ¦K}ˆ?ï莈)ÀÕ?g"íåŸK?gqwæ½K?g"íåŸK?îŽ{Aɵ?³ÒNyӂ?§O›}¯?³ÒNyӂ?îÝVžáñ¼?–ð)+º?¢*–¼ËA?–ð)+º?í°Ë!Úxå?£#Nª+8ó?²y¦ðPQÕ?£#Nª+8óAGN3FGL J1325.2-5411@s>¼¾aÏÿ@ ·;dZ¬À9AŒa¢²GÀ; èN2'ú?íñ—Ú;w@¥®¯*z}@Ì€•'¢¿Óÿúܪb¿ä=,°sa¿éX ÌSU¿ïÿÙ14*UNASNone@ŽdâmHPowerLawnone?ԕڿ¡¢?іZó¸ì?åµ /y¯?іZó¸ì?ÈþÐþ¾??Çð"%ØÆo?éÀKÀPp8?Çð"%ØÆo?åq*îÝê?³.§«¿²?Õª#ÄD,?³.§«¿²?ÙÞH†h?¨¤¶Íì?ã@qÛ¼Ì?¨¤¶Íì?Ç&ë,Ål?È!º(Êw?ê6E4Τú?È!º(Êw?¤Jõ²ú1Ã?·sÅ1%{Š?î»P¤™c$?·sÅ1%{Š?Õ/ÎzÝýÞ?»û{‹ç?åh'?»û{‹ç?¡¡ç)wü?…e\ÃRå%?îåîÒ °?…e\ÃRå%MIXED3FGL J1326.2-4651@sQÀ­Ú@/4ƒì‰*·À9ÕÜ@WÀ;0¥:·‹ó¿øÇ6þCè7@
²¨óSÊ-@Ž— <A?ïíȬýj¿ê¿«aB:7¿ïþÍë'MC?ïó
ƒ½²UNASNone@€"ÊŒL˜PowerLawnone?ïóžü7§?gmŸDó1ã?XÂù%÷³?gmŸDó1ã?ïÓ
‹k¥ã?ˆOú½kí?vzºO¬n"?ˆOú½kí?ñ¢Ö??–倮#/?¦·Àâc
?–倮#/?ïÿÿ(-Šl>¢Ï \™;>›…3>¢Ï \™;?ïÖӏšÎ^?'"sƒÈ?t–83H¼è?'"sƒÈ?ïB£‹s?°q:",u²?œ·«†Ë´?°q:",u²?윹'((`?ª{#¤Õ>?»3v¾½?ª{#¤Õ>?ïÿÏcÞZ?
bÖÍ6üá>øN¨4ã?
bÖÍ6üáAGN3FGL J1329.1-0536@sþà"'@LÆ)ñkÀ9ƹ#¢œxÀ;@2芘u¿Õ?Aì@esˆ¸Ë¹@Ð
€CR¿à'Z$—¿ã°q7!C¿ààAƒOw¯¿çt¯œ\¹âUNASNone@šþ•L˜_PowerLawnone?ïýhâ}ÊA?1.\U
?4¸í"[À?1.\U
?ï×b—Ï¿ñ?ˆ—‰;V?tN´0Ý7:?ˆ—‰;V?ïÎÝs80ô?sÄ~h'?x'F~ç?sÄ~h'?ïöó‰F‡›?;?ªD?Rí}?;?ªD?ïøIï@?RÓpƶ?Oóï|£'‡?RÓpƶ?ï9´§_?¬¾‹ĵ#?œXÉtò~	?¬¾‹ĵ#?îç0)­<S?—ÙPîÎâù?¡Œýh›ÖÓ?—ÙPîÎâù?ï‹@
óCë?€Ï°S-È:?/ürùO?€Ï°S-È:AGN3FGL J1330.4+5641@\
gbé@MТ ©XSÀ:dš,fXÀ;øwéE©¿¨Q&#°RQ@OƒNÿl‡@öê?yg ¿å,öŽÖâ¿î–56¿¿±^:íU/¿ä!q)búÌUNASNone@u_¿±[W?PowerLawnone?ïÿÓ­Å(F>ðÚZ▧¡>ö):íò‡/>ðÚZ▧¡?ïáê¼ø?'zÒRD?noåJÜïó?'zÒRD?ïÐ̞~°µ?'o¶üÁ?w™°°ÙqŒ?'o¶üÁ?ïöG—¸?@;øüיN?Sqù7¨ÿŽ?@;øüיN?ïÿٕ™@>ô{)g^ý>ó5PK$$>ô{)g^ý?ïAõáC&p?¥^0D½à{?—ÁCÏ,?¥^0D½à{?ïÐG‡†¥?{¯mà;8?wòÜTIñJ?{¯mà;8?ïÊɞ*^4?tô_q­Qê?z›0úŸ?tô_q­QêAGN3FGL J1333.8-4417@sn#9Àëî@1í…zþ£ßÀ9žs;`ÿÀ;R`ÊE3¿úœ¤cL*¦@ðwÆO@}þÿú̏¿èj!Ù­l¿ìFÂer ¿Â¹­åoÊ­¿ëÝg:UNASNone@ƒ"oiPowerLawnone?ïîJ÷Ü+K?`s‰ý~Í9?aµÅo?`s‰ý~Í9?ïӝ£‹Ø2?ˆaŽóõÆñ?v1.'k?ˆaŽóõÆñ?îù[Í"ã?"IÄmxk†? jC1+fÎ?"IÄmxk†?ïÿÖÖL8¤>ó?(d­'Á>ô"½—7³˜>ó?(d­'Á?ïîh…qæÅ?b5aHµÊ~?a—zÅû"?b5aHµÊ~?ïÑlCË?°SqkÉÿ?œ%Ò|®	:?°SqkÉÿ?îlÎĖ?ž`bÔ&+?©>GÅ?ž`bÔ&+?ïýȪu¬L?2k•'o?1º¬ðò	?2k•'oAGN3FGL J1334.3-4152@svçl‹C–@4K=áâއÀ:–ßY—KÀ;ºXVk¿ªmyÝ@
4yeqžÔ@

ŸzÚ¿ÃB¿­ªr°¿ïþ¯€ê(Ü?ïè÷·uçR¿ãîüúD³UNASNone@µÑe$ÝPowerLawnone?ïþ+óŠ?,tÁævÔ?-@Çëû9Ç?,tÁævÔ?ïÏfæÐf?ˆÍGÑj?xLŒŠçI?ˆÍGÑj?ïÒ;ÃS?ußdb
¥?vâ|F­z€?ußdb
¥?ïýoà?4Ì÷ᄎ…?7‡3ç_b?4Ì÷ᄎ…?ïüw2͘á??"$hè—?<Fk¿??"$hè—?î÷f˳iœ?²•C_ÖÂ? ‰"B5±G?²•C_ÖÂ?ïÂ[P¢s¢?~ۗ+²`½?~ÒW—h×M?~ۗ+²`½?ïùîïó~¤?[¥3ÿ''<?HDA<c­?[¥3ÿ''<AGN3FGL J1335.1-5655@sNSŽóMj@Ã֞ݦ9À9ŠÙã5ÅÀ:þIc `É?á¿0rþ>@Å0Pª½X@´8àœ7"¿ßî·§»_+¿åÚä_ð¿ÝQùX,M¿íö‹ÅùýeUNASNone@˜ZXbMÓPowerLawnone?îýèît?ŸØ\¯? .Ñq¾_?ŸØ\¯?ïis8ÜÀ`?œ`Ú¦Î7:?'јé]þ?œ`Ú¦Î7:?킱æl†?¢ãnºGäñ?³êpÎÁü?¢ãnºGäñ?ïCõÎ"ã/?uÝdÀŽþ?—F;£š$?uÝdÀŽþ?ì×¾\5?¼ˆ¬ï.C?¿g¡B
T?¼ˆ¬ï.C?ê×»¨.ª/?Ä%cSƒØ	?Ä¡_EWE?Ä%cSƒØ	?é¤8ëG?²S'ÿÚÑ?ËÁoS®å?²S'ÿÚÑ?ë£è±žŒâ?©r¡p=?Áp]9…Ìw?©r¡p=AGN3FGL J1335.2-4056@s|quŽ@5.©÷µ®£À9R%cf×¥À;Ov©ªˆÕ?ÉAy"÷@]EÀÔq@p[­Š<¿çÙ|Oa¿é㼊àCL¿å艧ÝÞ¿ÛnÝzUNASNone@EòäPowerLawnone?ïü¶V`+[?4Ú.ýöè¹?:MLðYù ?4Ú.ýöè¹?ïÈNßrR?8jw¡¦?{ؐB'o?8jw¡¦?ï²½ËÔ.?x¡ªd¹Z?ƒP4Ôœ?x¡ªd¹Z?ïÜ}´'m?V0­[;9»?qÁr¡Ê?V0­[;9»?ïöR¾OÐ?QZÌþ1/?SZƒ(ðã?QZÌþ1/?îj³ø•}€?µv²ØO¤è?©TÀx_õú?µv²ØO¤è?îÀ¬ÂãŒN?œæol<?£õ3Õ6×?œæol<?î/"òÞ?›EÄö¸°@?­Ï@K?›EÄö¸°@AGN3FGL J1342.4-6904@s7ÃAž0À›s¢¡À9§vÖöò:À; ãœòên¿ìÃ4ø@È-*Ûv@8¬Ë¿æöfÏþõ¿êô³|>¿ÚËàiÈ×±¿çج˜5&ºUNASNone@‰z¼£n/PowerLawnone?ïÃïW]¬?°5"°}k?~t@cmô?°5"°}k?ï¢ã•nÅ8?"¸ÎÐù?‡G®…ä?"¸ÎÐù?ï˜É1"(æ?"Þ	^n7{?‰Í³˜Žl?"Þ	^n7{?ïûæjO œ?2>þÔÞK?@fVIþ"÷?2>þÔÞK?ïîu/¬?fþZ)o"?aŠüj;d?fþZ)o"?ìò—þ?ÁÝ!¡Ãè*?¸k@Ő?ÁÝ!¡Ãè*?îïàë	EE?–þß!@Êÿ?¡ñQÿ`¥?–þß!@Êÿ?ï¾a ù—(?vXY""ól?€g·Ñhj?vXY""ólAGN3FGL J1345.1+1949@}Èû†ô{@RìÉ.À:?|èˆêöÀ;Ïòü~¹¿Ø†
á/…@mìðƒ¶@Ò.@Z80¿é…U;¿æa3æÙµ¶¿à¨'v'È¿åìb?vs¶UNASNone@"ÐrGE8ïPowerLawnone?ïÿ/XÃe?t8¶?/?è{c²?t8¶?/?ïیëá:?†Öé&çÇ?r9‰ò†<"?†Öé&çÇ?ïÐ]"·Šú?sIïv"¯É?wÑ6Ûë+?sIïv"¯É?ïön]^3?@9GíË/l?S"àû5?@9GíË/l?ïþ²þÎc?0– EH?$Ð>ƒ¶?0– EH?ïÚ=^ì[?±¸=Z?Ÿ¸K‹n´?±¸=Z?ïm{"W,?>QÌã°?'P›µ
ú{?>QÌã°?ïs×ñíª?‰ƒ$¾^×?'…AÂJÆ?‰ƒ$¾^×AGN3FGL J1346.2-2608@sà)~+V@A'Ó"vóÀ9êwXüñXÀ;³$™<|ˆ?è6'Ú!@‹£š#';@›'`—¿ä•ë8âí¿âÖ^¯§è¿ãR]ƒG¿ìÂ,G(*
UNASNone@Žh(¡ß¹9PowerLawnone?ï'ZršÚÀ?–Gñ:?›±±Ìý?–Gñ:?ïuC?¢]€¤*AG?¤ÞÄrÀyÉ?¢]€¤*AG?îo=`ÄÍ?(ìâY?®9)ó³/?(ìâY?ì Oû?•SÊFN‡¼?¿Öÿ7¥€$?•SÊFN‡¼?뜞ÍËg?¹ß_¡{:^?Á"Ë´Òc?¹ß_¡{:^?ã7A'"ÑÞ?ρƒ¢(?ّ|ûº\C?ρƒ¢(?ê´è%T§?°¸Àq2¾?Å,_j¯Ýd?°¸Àq2¾?×;üoý"ê?±š×¾y?äbÈ6?±š×¾yMIXED3FGL J1348.5-7150@s6t¼j~úÀ"î%¦'¶(À9¼ÚH¶RÀ;ZÐW›È?ÚÉN[5cm@@&=+""@€¥+ô¿èWt4¿êÉiñ5aâ¿Îž.bج¿æêÜØ2±ƒUNASNone@"†)~+VPowerLawnone?ïý‡‹‹J2?J¾­ù]"?3↵z0?J¾­ù]"?ï‰s̀v³?™rf€p?£ßâSG?™rf€p?ïݦËþ"?j«ENì?q,šfd?j«ENì?ïÓ§|mÂ?Y¹Ì.˜ú?v,y¿	n×?Y¹Ì.˜ú?ïú¿Ñ^#n?MZ‡²±‹b?E¹úµ{?MZ‡²±‹b?ëì2/ýô?ÂHÈ_™‡?ÀO7@-Ì?ÂHÈ_™‡?ïeveH?p?Õ»ì|Uì?"Q3Zg­ù?Õ»ì|Uì?ï(R»Óo?+îÎÝѵ?šõ¨ƒÚO?+îÎÝѵAGN3FGL J1348.5-5833@sezÁҝÇ@ß°&£Ø¸À8ô´JÀ:æ$óÅ?´¾ÛÚ.@âøc!@XKŸ©†¿êL:­>ÖÄ¿êYãñ#ǿ׆£˜ÞÖ¿ê¤{X™}UNASNone@}a=1¹¶PowerLawnone	?ïÁí¾4¼?ŠJÐ'z?	 Ø@2?ŠJÐ'z?ïx×úþ8€?¤9,ÛûõÌ?å™Y¸?¤9,ÛûõÌ?îRÆvqve?žS¥ßòD?ªÓ˜™Ä€±?žS¥ßòD?FKP,á?fï6Œ_›…?€Öm.uô?fï6Œ_›…?ïGB‹ã?¡9"¤¦ä?—®‡ZI?¡9"¤¦ä?ë®ú/l»P?Âô#vhM?ÁDBM¿?Âô#vhM?ìѳŽ?¬'ÿ+а‹?¿÷9rg{?¬'ÿ+а‹?íåFÀ'#? C†UMa?°ÕËC è? C†UMaAGN3FGL J1351.1-2743@sì^_0çÿ@@§T!ÀD(À:¿¦¥òÀ;šCV–势öÀ)æ®JV@!¯B"dY@c cbP¿ÞI]褪ֿì?ž8dË\¿äóC¶……¿¹~"d%EUNASNone@•5¡ÊÀƒPowerLawnone?ïþ}áy¤~?(IÁ*3æ?(!åd¢t?(IÁ*3æ?ïÛ`Í	?'ÂõµÝ¯?rOó»×§?'ÂõµÝ¯?ïÁQº:?t¿°½ù#†?W"ü,T}?t¿°½ù#†?ïÿö}ÓÈó>ʂ;˜—>Ó¶M>ʂ;˜—?ïýŠÂÄ<?6ïÔ«þYŸ?3©î;Š'>?6ïÔ«þYŸ?ï<ϺE"<?«åj4sœ|?˜f¼tâk?«åj4sœ|?ïúâðá»?–%yô3?à£žt,Ÿ?–%yô3?ïÿÛ2ãz?! þ*Æ£?$U%Ja?! þ*Æ£AGN3FGL J1351.8-1524@t;Ýcˆe•@FZ³R¨À:E{°z†¯À;•
ùXF¿ËùÈä
4@Ğ×F"y@4`JmŒ¿ì¬ €Ò[¿ãçäeI¿â`ÇúfIF¿ÕùÅÈexÄUNASNone@"àžì¿±[PowerLawnone?ïþèe&â?¨rà,XJ?!y©…¢¸Ù?¨rà,XJ?ïØEÌã?ˆ8ë‰|z?sÝ~IÖ¾‹?ˆ8ë‰|z?ï×ÂõTù?s­vÃ[†?t~ž Òc‰?s­vÃ[†?ïýQ¦Ÿâ? ÿð䀑?5rËȺÂu? ÿð䀑?ïþ‹|("<?&óì´9Q1?'H9Òà¤å?&óì´9Q1?ï!ª
fF—?­-/ž_C`?›Ê¾¶¦É?­-/ž_C`?ïp1Ñ×?Ÿs'—?'þœ±.¿9?Ÿs'—?ïÞ
À­¦?g1|ÐdJ?pùú8ñ.?g1|ÐdJAGN3FGL J1400.2-2413@t&©Ür\>@BÖ¡aä÷À9ÞvlmçdÀ;¤ñ-À?ó¨›C@U;ÉÇ_@@Óàx"¿åÞ÷*T£'¿Ñ²Å1u¿äÈò¯3<¿ïÿúÐÚè2UNASNone@•WV»˜ÇãPowerLawnone?䙨g蜌?ÖC'+f5>?Ö̯0.Æè?ÖC'+f5>?á'ºÄ?ÉôXTÞ\J?Ý°ŠwùÇé?ÉôXTÞ\J?äþO'ã?³Â‡æ̳?ÖaÔÜ;?³Â‡æ̳?âCÀ"È"Ç?ª>ðå¬?Ûx~önör?ª>ðå¬?יð"ÈÁ?ÕZÔ,<ží?ä3¶Ÿ2?ÕZÔ,<ží?Åd«c¤Þ?ÆH]ðSÃ)?ê¦Õ'øÉ?ÆH]ðSÃ)?Òk)À)ë?º;
6
Fÿ?æÊktë?º;
6
Fÿ?»ü;¶u®"?žÔ¤=©²*?ì€x‰1J-?žÔ¤=©²*MIXED3FGL J1402.7-3240@sþ=ÈK@;ØÃÁ‹P+À:-bŒ½EÀ;´ê8v¿×wò.J@Ìdȵ@‹\@r¶×¿å*±Pg¿ç`ƒ<ØE¿é7ÞS¿âçƒ(áUNASNone@‹fƒFÜ]dPowerLawnone?ïýAn?<ë?<èïT?5÷ e»xs?<ë?<èïT?ïÓèw?ˆkm9ÓÜ?vô{ ?ˆkm9ÓÜ?ﺋ[GB?s¼"û:?Œ?])H+‹?s¼"û:?Œ?ï÷ƒh;?;jsl=v?Pù/ðx-?;jsl=v?ïõªÕߤ?\ñn)ÄÖ?UÜ©ô©L?\ñn)ÄÖ?îí'è™?°x8ÞF[?¡&áuŽ=?°x8ÞF[?ï)æ-úlÌ?"X@Qârg?šÃ:D""?"X@Qârg?ï<ö8p?ŸÅ߁?˜a>õŽUü?ŸÅ߁AGN3FGL J1403.1+1304@vH'ýuâ@Q—á2µ_À:Ájî‹À;ïQ{×?éüQ·Øžè@ÄîÕÒ°@ +ßVè¿äÏì‡cr¿Û4¸#G'Ë¿è|&x¿ïÿ"¢[VŠUNASNone@"NTɅðPowerLawnone?3&?¯¬OŸgžQ?¤Ö|Еl)?¯¬OŸgžQ?í—N0˜+ä?±sÇ»Ûü?³EŽ{¬"`?±sÇ»Ûü?ë+d×½c?ª(¬>ßO6?ÃRl¡
s™?ª(¬>ßO6?ê/Ä ¥ÉË?£¯…ßÛü?Ç@í}hØÔ?£¯…ßÛü?ì Qûå?¿9æ"¾¨?¾ýp ×ïs?¿9æ"¾¨?àœÌ//Ç?Ñ(ƒØÎI
?ÞÆg¡ r?Ñ(ƒØÎI
?äÖÒe¤/Ü?¸XoíŸ?ÖR[4· H?¸XoíŸ?ËÎ@—l:2?±0ÑÐ÷çž?éoÚ$ñs?±0ÑÐ÷çžMIXED3FGL J1404.3-5241@sŸ¬1&é@!4úïõÆÁÀ9²ä¥5¯À;I¼2JÕç?ê­-°Åã­@ޒr@Щ¾€¿é½«û#«¿ÔÍ6ŸNdg¿ì/¤`p¿åL²Æˆ²UNASNone@'‡aÊÀƒPowerLawnone?ïjšµoÛR?š(Èç‰m?'¬©R•Í?š(Èç‰m?ï†d¼ß?¤0N·ª?Ÿ3kë ?¤0N·ª?îÊȪmF?"¾äó-`?£Su[Â`?"¾äó-`?î64Ô¦"?Š<BäFµ?¬Ÿ±Ù¯É?Š<BäFµ?瀤(z?ɉtŽÀ?ÐÿÜ·¯ú?ɉtŽÀ?ã¾ Ís"?Ð
ùhóDÂ?؂¾eÎø?Ð
ùhóDÂ?êfISÂ0"?®Ê¹]Ž?ÆfÚ°÷?x?®Ê¹]Ž?â'Z'`9?»ˆÌŠæ+ ?ÛàÝK±??»ˆÌŠæ+ AGN3FGL J1404.7-5844@s…d2‹n@Ki~J‰À9ªÂ©][üÀ:ÍçâÒÉ?І5lQ@
Y»~Ư|@U]ŸÃTS?ï=p?qô©¿ìñ£êƒ¿ãv˜@[ÿ¹Þ'$¸ÏUNASNone@·kÁ×ÛõPowerLawnone?ïï@_£\?‡\ÍH·"?`¿ø'>[Ñ?‡\ÍH·"?ïxðJð ?¥¦A£²xî?áö¡ÿ¼?¥¦A£²xî?ï# ½
ž%?"Í2Ì{±6?›‹èV5q?"Í2Ì{±6?ïôø҆—?E&Hÿ"?V[B‡î-?E&Hÿ"?ïß%óë°Ï?€Øæ7	]?pm
—4"?€Øæ7	]?ìE£ÞAq?ÅÞp}?½Òá
÷d{?ÅÞp}?îMm\,"K?¡‰Qf¾À?«)*Aƒ>J?¡‰Qf¾À?h4æ?2#Øf!â?‡eèª2u?2#Øf!âAGN3FGL J1408.0-2924@t%܇Tó@>'Z³R¨À9®`À48À;±£|qk?ó13ú-ƒ@pù½EÆ@|¾`xe¿äÂÛ­÷ZÑ¿ê(߀6NÏ¿ìû+–¿í»ÓáûvUNASNone@z3Âã?PowerLawnone?åÖü9¡â?Ç~Lì¶s?ÔSŒ¼<?Ç~Lì¶s?Òkžã»?ʲX%þ9?æÊ0ñöŽ"?ʲX%þ9?ë;-ìwb?§é¿Ä??ÃçHN"x?§é¿Ä??Ú2ªFÓ?«]µ›då?âæªøwܗ?«]µ›då?ãâG³Gë?Ì2a–""?ÙÖ;p™p)?Ì2a–""?´-MèïÓ?Â6¤#F'?ízVCK?Â6¤#F'?äôØw$ú‹?¸pÁŠÙ 5?ÖO¶
é?¸pÁŠÙ 5?¡ù¸í`¯Ý?Š"BÚªŒÚ?îàdpå<Ó?Š"BÚªŒÚMIXED3FGL J1409.2-3743@sø!-w1@6¢DAxpTÀ9ÂÏL
ÑÀ;•e×y¿ïݦXނ@1›Â"¸Ú@—Iÿ¨lE¿ç<Õã™9o¿ä•ìÐj^¿èPâèÂø¿ïÿ‡{£©,UNASNone@|Óû½{ 2PowerLawnone?ï§;ûÑâ?‰.	å7ü?†1>óMŸ?‰.	å7ü?ïÑè¨ÓüÊ?‡]˜#²=©?w«ˆC*Ù?‡]˜#²=©?îl‹h Ê³?–\Dà•è›?©7IumÖ?–\Dà•è›?ïø+"àqg?A _´3î3?OQì«Û›?A _´3î3?ïZ‹"À?¡¶x1öåS?œô®›¼è?¡¶x1öåS?îô]7=®â?°œ£d¶g? º,‡ÙŽã?°œ£d¶g?ìµ­‡žV?ªÓb²å‹"?¿ZR"Ã
S?ªÓb²å‹"?ïÇ)Ÿ¶"?•Ä}ʂ±?Ÿ'Ñ0—t?•Ä}ʂ±AGN3FGL J1410.9+7406@\ﰉ 'R@DòF¿2/À9›ÖøjÀ;ûœGÉÃ-?ñ(ÆGÍt@.rÆÆù@Q_Vý"¿é÷£Öâ¿âEu³"ô¿Ô?Èå.þ¿àOœ&€ŒUNASNone@–V¤tSŽóPowerLawnone?ïà²À12þ?vžN\ËÝ?oM?¡r*f?vžN\ËÝ?íŒ2Ài¥?¶	œ0k›?³žiûmà]?¶	œ0k›?ï(¨u×Ú?"a½Ð©§ä?šêÿï6Í?"a½Ð©§ä?ë¿´ôÍ?l¢qÇ?Á,/³ÌÌ?l¢qÇ?ᅩ§®_?ƒ'(3^?€ÖMr°<?ƒ'(3^?àûˆøj=?ÐMæ•ÿ8ã?Þî+…Ú?ÐMæ•ÿ8ã?íÞ' 'ìÚ?¢Ì=r¾Ì?±Âûè™1?¢Ì=r¾Ì?ÞùÒrßq?»ºh"‰¬‰?àƒÆýH?»ºh"‰¬‰MIXED3FGL J1411.1+3717@QFȟ@¢‡@Q—hƒöèÀ:nêžnëpÀ;ü jÓ?ÙÛ3tì!@
¾¤B¿î@ÒäŸý5ö¿évâ0Ðò¿è×Ýú#k¿åÈ-§iL0¿ÉÛ9B†UNASNone@ŒŽæ">jPowerLawnone?ïþ;g½²?:ïcÖ?,I"N§·U?:ïcÖ?ïÝ«7·ãm?"Žü!—ã?q*dDZd?"Žü!—ã?ï¸3ÚfØ?wá}Y'2a?ó	`ʚÁ?wá}Y'2a?ïØns¦ý?aƒÚv É£?sÈÆ:³ñd?aƒÚv É£?ïôõêõ¤)?eFw}7?V)ž¬?eFw}7?îªâðá»-?±mbvE@?¥QÐît±;?±mbvE@?rˆfI?  F̌?¦gxØU'n?  F̌?í¹6jJK©?ª€R¤&`H?²6L­?¯<?ª€R¤&`HAGN3FGL J1411.4-0724@tñ ä¶1@I3]9—À:†ÖHv'À;³c"GÁ¿æ¶twºæ_@ñGÊDj?þ]Û O@Z?¬U#I»?ᚌF'Š;¿â¢át';¿Ñ-•ÇIwUNASNone@³"j~ùÛ#PowerLawnone?ïý–&ٙË?0H%bÈ`?3NÊËßs?0H%bÈ`?ïÙ;›´"?ˆ8Ûq]îÑ?sb2zÕ¡ñ?ˆ8Ûq]îÑ?ïɄ]Ñu?uÑf‡™÷î?{=ÿ»É±›?uÑf‡™÷î?ïþàoŸ~? WD"õ·?.¡ýø"ù? WD"õ·?ïú›mú"?Câ{kq±?E'JæpFk?Câ{kq±?ï/èÕ/á‰?¬'µÝ?šåTÜdë?¬'µÝ?ñ<?†2Ôüa³ü?ˆûÔ9b(<?†2Ôüa³ü?ïàïAýâ€?kTFÙü0Î?o½Û¡à"?kTFÙü0ÎAGN3FGL J1417.5-4402@síÒܱF_@0&s>»ýrÀ9W€•ÓÀ;h"¡T¢?ؕ0›JÁ@&"~…@óQŸÚÑG¿ä'DˆÆ¿¿ãò[/Y=¿â{Ë¡dÐJ¿îØv°zJŽUNASNone@Qœàu÷PowerLawnone?ë«4š#ñ?½¹äìíîI?ÁS-—›p<?½¹äìíîI?ï'g:µ?›<J=xÌé?f1x£à?›<J=xÌé?ëF"Gp?¬2¹ü°w?Âå²â?û™?¬2¹ü°w?
T(?ˆMÊëØ3?§†Ÿ\uM"?ˆMÊëØ3?â/—+oe?ÊãҚ8M?Û Ñ©!ï5?ÊãҚ8M?êÃþFa®?Äýï#䶣?ÄðçêyJ?Äýï#䶣?âJ5$ÇW?À«´0@1?ÚÅk•¶qR?À«´0@1?ä$þ¼D%?·?Ù	úˆ?׶À‡w·?·?Ù	úˆAGN3FGL J1417.7-5026@sËË)^ž@$9¹×ý'wÀ9u΁eÆÀ;7E¶Ãv¿í‡‰½AZ@
­^܄OÛ@âZߟO¿ë!ǕLÐ5¿áuV^¹ýE¿çMe—¿á÷¤DîGUNASNone@Žjô¢3œPowerLawnone?ïåv¦>\v?n!}
½'N?j‰YâŸÉì?n!}
½'N?ï¼í‹€ž˜?"®Súß?€Ä(mì?"®Súß?ïPHÍyE?ˆÎLW08c?•ýöݹÑj?ˆÎLW08c?ïý"v"ÜÆ?%R"¶cA?3dI==–?%R"¶cA?ïX+Á›?"áÑÖ$ç?"ú‡ã<9'?"áÑÖ$ç?îj›tBÑ?¶×ªå0Ó?©XI—¹ö?¶×ªå0Ó?í‡áí°?£)^ˆ¡y¸?³À𗘆?£)^ˆ¡y¸?ᆭá֟4?xZùÐ*ð?€VG‹¸?xZùÐ*ðAGN3FGL J1419.1-5534@s²³œ¾à@Ê'ÿÀ8Úoõ—ÇÀ;õ€J=;¿éݬý4Û@ÏJ€Æ@‡·ßªÊï¿ê˜úpQªJ¿ê~­øvHÝ¿ãèw¿êÛqÒò´UNASNone@wyfšÔ,=PowerLawnone	?ï½eïYP?"£a}û+Ñ?€»f|B'?"£a}û+Ñ?ï±þîï?ýˆ-?ç?ƒ¿€I¬Ê?ýˆ-?ç?îOÝ]
>•?å¢¢%'?«*.€/¶?å¢¢%'?ïûxşÃ?3´æS=.?BéÍ^D^?3´æS=.?ï'K'ÎÉý?–þ3ô?m{Œ¤?–þ3ô?íãD˜?¼LÒߔ_?°ãÔ=?¼LÒߔ_?ëâïÚ ¥ð?­¶ð£;?Àt@—}h>?­¶ð£;?ﰂóԒX?yZρújç?ƒßC"?yZρújçAGN3FGL J1420.9-4615@sê±[W>«@+¹ò™0À9'Ùe5À;i@։äñ?Ð'ÝßÄ¡/@
Á¬œU¶–@›¥^¿ÿ¿ë"¶å@a¿æñQïê¿ä3½6¬º^¿êÌádßR¶UNASNone@€­!ÊÀƒPowerLawnone?ï¶p¹óΑ?¶=¨ÒӔ?'cÑtÿä?¶=¨ÒӔ?© þ±?š"Upõ¶?ŒÐ•­qÚ?š"Upõ¶?ïR—L¸?'*¬{ôm%?ŸÕ¾c?'*¬{ôm%?ï´nuî3?~âaϟÛ=?ŸIr-ҝ³?~âaϟÛ=?îðɾqâ"?¤FZÓZ8? ódáÖÓ?¤FZÓZ8?éßÁHV¨P?É0.ív;?ȀúÞ¥^Á?É0.ív;?í!º'z«?¦'k?ª?¶ò+uŽÑ?¦'k?ª?åÁ÷Oh"4?³û+³¹µ¬?Ô|a.÷˜?³û+³¹µ¬AGN3FGL J1421.0-2431@tzzcslß@A¿"ÀiÀ:…îÁêÀ;²';ýP?ìPó/›@Mk›Y:@šÂ?U*?àZ¶_ևê¿áü»yµšù¿åÀ/@Æè¿ïÿ÷,OqáUNASNone@–+Ã{J#:PowerLawnone?êÓyʶÈ?Ïg8w¯}Ë?IJÕ$à?Ïg8w¯}Ë?êK®a?¿š"¯ÇN?ÆӗµF{î?¿š"¯ÇN?éQQŸëÿS?°WZ½,?ʺ¹€P³?°WZ½,?碲ÕTÛ¥?¦Pìâ¹?кšUVH·?¦Pìâ¹?èµ@"Ó?ÐéÕöZÿo?Ï¡*ý¯˜´?ÐéÕöZÿo?ٟ6£Íq…?ÎùÌl!2Í?ã0d®G>?ÎùÌl!2Í?âSØ=T…z?¼ê9`ÉÄ?ÛXO…Võ
?¼ê9`ÉÄ?Êòy¸0f?¨`Løe?é|a'óæ?¨`LøeMIXED3FGL J1421.8-7920@s3.œË}AÀ1;'`4PÀ:0«ÆÂǐÀ;¨Ò3>î?ð™@Ù9Í@0Ç˱ç@&@tdV?î àç?¿äªÔÚ.×{¿å½'T«ÓÙ¿ê«';…UNASNone@I=ó¶E¢PowerLawnone?ë|î—ð¤?Âû­Óë؉?ÂE ?q?Âû­Óë؉?êlâiø?Á{›ÑF
?ÆLuúX ?Á{›ÑF
?ìŒïŨÊ?«Ñ@µ2ïo?¿Ã˜Ò¹²?«Ñ@µ2ïo?éÇáü'jÚ?¤}…"c€¬?Èàx
¶T™?¤}…"c€¬?ä¼)½yÙÇ?Îv™u˜™¦?և¬…Lr?Îv™u˜™¦?Õ3òKó"®?Ï8
ýàZ?åfÚ=©?Ï8
ýàZ?ÞÖ̵¥¾Á?Á(5•Ûkn?à"™¥-  ?Á(5•Ûkn?ÕýW
Ë,†?´N0ìÈDò?åTzši½?´N0ìÈDòMIXED3FGL J1424.3-1753@tÁëíúCþ@CԍûÖ¥"À9äZ#bØÀ;¤Wë‰P¿Ún,£¢%@1s0Ï*Ë@c]a#Ü¿é\~éjl¿ß'"®iÏ¿ÞÆÁk«ÛÍ¿á§ù´"û-UNASNone@šóÎ_PowerLawnone?ïþ0ôOÚ?/Iw&¥ÿ?.<ïŸU؉?/Iw&¥ÿ?ïÖäñºJ?ˆcè¾q ?t‡›¡®?ˆcè¾q ?ïã1á'(?lÓÃ3Ò?lÎSK°C?lÓÃ3Ò?ïúàÚ(ˆ"?0}'¾ƒ?D|—õ§?0}'¾ƒ?ïüçMÆKB?5øhµÚèÉ?8ŐP#?5øhµÚèÉ?ïU{1¤"?­Ÿ4vÜ?œ5P'ì5±?­Ÿ4vÜ?ïÙ{|8,?xߌuJV$?sB}65=ô?xߌuJV$?ï·ô­³ÏG?uý'£Dï?'Ô¢Úb?uý'£DïAGN3FGL J1427.2+1610@'.'O"}@PPe¾ ºÀ:¤.™À;ÅÏASCÀ•Öé±4@;cÃÉÃÙ@O?ƒM¨¿ê/¨+º÷¿èƒžNEn…¿æ‡iJ"Äe¿ïÿqñp+rUNASNone@rÕºÇË)PowerLawnone?ïúú®Ì˜?AX¶*ç0?DE‰ß£õ?AX¶*ç0?ïã̈́O&ü?€2áÔCØ(?l2{ÌUãÊ?€2áÔCØ(?ïêõ'úÕ?'Ë™˜?œ¡OXsX?'Ë™˜?ïÿÞÎñ®ó>ë C#W>ð˜fÐJå>ë C#W?ïü¶À#¤¨?;¯µ,­??:Jî8Ó#?;¯µ,­??ïX"ãôu?¥³Û>
Å?"ÿ› ÕV?¥³Û>
Å?ï&³þt»?"!ä¸C+b?›?	‡ ¤?"!ä¸C+b?ïúÐGH?IÂ䢰@ü?F¿ó'×ñ?IÂ䢰@üAGN3FGL J1430.8-4434@t'œàu÷@-•Ã½Y'CÀ9"Ü%/drÀ;nú|2€†ÀknY$	@ø¼—u}@Í?†'Í¿ß×ólàf¿çIš†\.¿ÝvÑӜʧ¿êYIä5Û?UNASNone@"#Ê#9ÀìPowerLawnone?ïßiF‰;? ½gØks?pK]ˆöB? ½gØks?ïҋ'w
›?ˆaŸ­.÷º?vº>Ɗv?ˆaŸ­.÷º?ï^¡0"N?Šá;Õ+1?"+Þ¢"œ)?Šá;Õ+1?ïÿü4Ìîä>ÂæԆ¹:>¾X»èÊÀ>ÂæԆ¹:?ïÏlzžú?zW'Œˆ(?xtI°"Ÿ?zW'Œˆ(?ïm_)]?°£˜+Gê?œòTm?°£˜+Gê?í¸¢´ Ë?¢lQÉ?²:ï2Zù©?¢lQÉ?ïÿy¶
ª?=|Áeºb?ÉFÁ?=|ÁeºbAGN3FGL J1431.1-6425@s—¾ß¤@À؅Ó7ëÀ9K¼šO¡ÿÀ:þ¹™aÝ?æú¬ä•T@›5sñ@»Ÿú[Ñ¿æWþŽ]GÑ¿ê|˔WT?¿ãÀ+Ê^3¿ïÿÜ¡"œZUNASNone@"l¿±[WPowerLawnone?ïé~ˆ5
?pƒh¯ˆÅ"?fwåû3?pƒh¯ˆÅ"?îµÝ""Ð?®ÃSÇd?¤¢/5êËû?®ÃSÇd?î°9t'¿?—	|U'?¤üh»"/?—	|U'?îiÛ*U
–?…¯<{ØÔÈ?©bM^òž?…¯<{ØÔÈ?ïÇ+ ö7Þ?†‹aÁ'¼C?|j/jB?†‹aÁ'¼C?âՆªS¦?Ì~•«½!x?ÚTò«X³Ë?Ì~•«½!x?ìÔŠ0ù{?¨78ÎÄò?¹_Û¯T)?¨78ÎÄò?æ[Üõr}?´Â®zå?ÓHFõ?´Â®zåAGN3FGL J1438.6-4209@t5K}At?@0lˆçš®mÀ:
xë¤(iÀ;fûéðÊ?ä	©`¥Ì@+-Ïqï@'¸`.>¿ílŸæe¿ä½4ºƒ¿ÙSÞ%²
¦¿Ò¨"^F\[UNASNone@ìÙè>BPowerLawnone?ïû…–q4å?E2»ûëJ?A馬lVà?E2»ûëJ?ï¤mÈ'?"A37F<?†ä¼ßm.?"A37F<?ï§å|—?'À]"¹î?†¡ˆ,<?'À]"¹î?ï
2˜"?p¥1'\/?‹ú|ÁO?p¥1'\/?ïéÿ{Sf?i¹+8G¯?f"Ã÷K´?i¹+8G¯?ëFL¯Iô?Ç``ï?N±?ÃêæÍBØ1?Ç``ï?N±?î/‡Ÿ,g?Ÿ÷Yڂ¤?­w†
9"?Ÿ÷Yڂ¤?ì‹J"襤?©#IóHt~?»¥«Ø'ÚÞ?©#IóHt~AGN3FGL J1444.0-7033@s'ÂzcsÀ#r-"ÁÀ9æÆ:"‰À;™jZÀ†<¶¿š4@
u_þmY@–­ _¿æU¶ëè=¿éDT@(4¿Õ$8܌ֿê-h(»éƒUNASNone@Œó思IRPowerLawnone?ïðrº˜ÓÝ?eáiÒ*©}?_ŠUfm?eáiÒ*©}?ï¹ñð6£?†‹$*?ƒƒûö!¯?†‹$*?ïOÅãØ	Ê?X²<¶fD?–C"þÆ´?X²<¶fD?ïÿþ¦AP`>²ŽŠ™>¥
;£ >²ŽŠ™?ïáá1ßÈ?s¡ØÙV?nÏ¿¡?s¡ØÙV?íõ0¸Ñåˆ?»¨N	ŝü?°Vz7¹Ä?»¨N	ŝü?îوEø÷g?—+$ñi?¢g{Ÿ"¢'?—+$ñi?ïÿÎdQŽ=?åY˜†b>øÍîÖ|&?åY˜†bAGN3FGL J1445.7-5925@sÐKÛ ¥'?ÑèxD4b]À8¼~Ù$À: ^ØP?ґ£¥zè@
~p+—@»;\_¿ƒ‡éÕY€Õ¿è%D
y‰6¿éW"#žô*¿åc}äd÷"UNASNone@¢öz¬1PowerLawnone?ÖïÆ°í·î?Ó>¼t¡"á?䈧‰$	?Ó>¼t¡"á?ï%d~WJ?±}oz›®?›Sp3|€Å?±}oz›®?âcNw˜y?¸å!1.õW?Û9ÙcÏ?¸å!1.õW?ï|¢(¿?tº€¾Z.ý?k»»`?tº€¾Z.ý?ºV?Qπ†?À¼êÎâÉ?ìµ8Æï?À¼êÎâÉ?èw²FÂ:?ÉVÏýPD³?Ϻ!6ä÷?ÉVÏýPD³?à‰˜"Ý5â?¹Õ9"˜Ý?ÞìϺE"<?¹Õ9"˜Ý?êbVðý?°¨¸ß±¶.?Æv¥È?ä
?°¨¸ß±¶.MIXED3FGL J1457.6-6249@sÌn—OßÀ2ô™špYÀ9;ÛmiÀ:Ú
>¬ãù?ì^bq`@žžô@™G€r+A?ïË&´A2¿äI
¾À«½¿íñÛØŠõ¿àÆ\_SUNASNone@êãˆe"¯PowerLawnone?ëÍfÑ"û`?Åþ1
†c(?ÀÊd»t?Åþ1
†c(?çÿ¦d
õ?ʛwú&f
?г7êø?ʛwú&f
?ì&p
?§H»m›?¿×æË®?§H»m›?꤭@¾?­æŸDŸu?ÇÑmKîý
?­æŸDŸu?æ÷v9uË?ÊÑ·ÎÁw?ҍiÞ?ÊÑ·ÎÁw?ÆW†! A\?Ŕ™Ï
]¥?êjw—ï©?Ŕ™Ï
]¥?ä†ÒKß?¹Gc1亻?×ÜóÒ[hB?¹Gc1亻?Ñ]lk§Ý™?ÂourŒ©5?çQIÊ,4?ÂourŒ©5MIXED3FGL J1457.6-5355@t÷zö@d@æK©K¾DÀ9™'W«¸€À;	……`ý?ÛIÝޘ¸@
1$¢e@Y^ðá)¿ç|m(CãQ¿ëݞc­Ï\¿Üb–#S¨Z¿á灇»0ÿUNASNone@•h	 'RTPowerLawnone?ïê˘oM?€!L7Zo?e4gk—#X?€!L7Zo?ïi©¬-½J? W¤0ë=?'ÊÊoÀ»? W¤0ë=?ïYŸwÃÊ´?¦–N­Úf?"Ìeák?¦–N­Úf?ïRãÊÊ?jJÊΜè?ˆ«G
}
"?jJÊΜè?ïR7¡ÌC? (ø)™lÓ?•¹kÆwž? (ø)™lÓ?é7pPŽÒ…?É$ÒÕó?Ë">½Äµì?É$ÒÕó?í%ýƒà?­]\SGc?¶ÐßH	
?­]\SGc?ìÍԝd?¤\ˆ Æ*?¹'[ÀÆM?¤\ˆ Æ*AGN3FGL J1458.7-2120@u)u\)@@JŸ±À9­—1àLÜÀ;•ÈFUNç?âƒJEžp@†úc
@»Å@;"e¿äËOT"š7¿à®îaᶿåí?}̒¿ïÿ°yÚâdUNASNone@lPowerLawnone?íuáðÈ'?¸bè¤Q?´Pð€­¥Å?¸bè¤Q?ëÛx¸3ÉÂ?»Ðô5С?À'0Ø÷?»Ðô5С?뻄řt'?§ãpWtê?Áìéš/c?§ãpWtê?è>¾veÚ?¦•ü–Ž?Ïž&h—?¦•ü–Ž?ä©ÍJdìØ?Î@¾"ÝG?Ö¬ek6&O?Î@¾"ÝG?Ø;'p(ÔW?ÑìgD"?ãâlGë•Õ?ÑìgD"?ãÇlÙ;u?ºhª+•¸—?Øq&Mlj?ºhª+•¸—?ÂUtjyà?¦pF³|¼?ëê¢åaˆ?¦pF³|¼MIXED3FGL J1502.2+5553@W2>BZîc@Js,­'À9},²æqºÀ;îW"KS»À	úf9oã=@‡Þ@ª£ +²¿å9_¨Þí¿èëBó^uÆ¿áÎÒǞ̿ìOq4ÿUNASNone@€/m­ê‰PowerLawnone?ïþ†Ÿ'3\?;õ{Ç%W?'–û§³?;õ{Ç%W?ïå1áµ£L?€ð>*Ué"?jΊõ[ö?€ð>*Ué"?ï´í#¾9?'ZUjü\?'Ä·)ú[Æ?'ZUjü\?ïÿÿ䞝>rë®IÕ'[>kb¡Û#¬Ú>rë®IÕ'[?ïÿšÇY'?âb1-¹E?	|]Ÿ'?âb1-¹E?ïl>ùÔ±Œ?¡™=£*B?'x ¾Š–|?¡™=£*B?ïàÝyÜÿ?vSWÜ°þ?o"…ñ†•?vSWÜ°þ?ïÿû…Ç՗>ÏE,ˆ—õ>Áé' S¾>ÏE,ˆ—õAGN3FGL J1506.4-0340@v,ï~=Á@F•´¢3œÀ:$³ÑSDKÀ;}fÿéYË¿Ùœx,r¶@
²…-Hc@ªyßêᶿà¥ÿEÅÜï¿ê^k¶Œ·¿àÑ@ÃzÏ»¿âaZÿUNASNone@˜Ž;Í5¨PowerLawnone?ïÿàòú?8Ró¤¯ã?á}øÓì?8Ró¤¯ã?ïÖ9`Úòf?ˆ‰ìXė?tãO©ä%?ˆ‰ìXė?ïÅ,mNë~?wç ¶Ÿµ?}iÉXŠ@ò?wç ¶Ÿµ?ïùXMçß?5a
à¾?JžË´¼ÎÏ?5a
à¾?ïþÛÓ%•?'Â^V2d6?"BÌ3ˆP´?'Â^V2d6?ïßÂ?®‰êc­ò?ž|}ß;Õ½?®‰êc­ò?ïàH Ÿ?–ƒdÍ)Öø?žƒööë$?–ƒdÍ)Öø?^\E•?p+b䎦?Š](s=n³?p+b䎦AGN3FGL J1506.6-6219@sÞò<ÈÞ+À¹§Áz‰3À9g´ör2À;¼(ßó¿ÔZë´æÉ@>—Îé2?ýµ¿©M¿ï»;µÀó?á<¶(Æs¿Ýª6˜K‹¿ÐQ¯ÝJ?âUNASNone@ºÎÑ·PowerLawnone?ïò¿Zsi?d	F÷r/?ZK[&y?d	F÷r/?ïV†¹0ý?žð«µ'?Œª^_r0"?žð«µ'?ï¡@%£ÂV?…›Hå.êå?‡¯ö¡^>b?…›Hå.êå?ïûe ‡ŽC?1jfv™{¥?Bi~´–£?1jfv™{¥?ï¾o='J?^<kT-?€d:à!MŽ?^<kT-?ìz¿ó0Êß?ďœW[}÷?¼*fy©?ďœW[}÷?ï1EP}W*?–›Aе?™×Uç¾Î?–›Aе?ïҚíÉÔ?l¶'Bk?v²‰|ÛeÉ?l¶'BkAGN3FGL J1510.2-5754@t›'·þ?À›ý6¡ý–À7Ûx\2/þÀ9öð{þ~ ?âÍ'æxð@™3& !@'qàBŠ¿Îh›!%‹ø¿èˆÀa•­b¿é8©F຿è"x±OÚUNASNone@''»/ìPowerLawnone?Ñ!"þm?ÏQšî>±?çon€øI9?ÏQšî>±?îü÷"ä'«?³¦§¥{? 0†Â'¼O?³¦§¥{?Úör
ʪ?¸o¢_œåØ?â"Æùªô?¸o¢_œåØ?﬌K¹x?€	è¸mö¥?ž
n}hô?€	è¸mö¥?ÊÝxƒ@ß?ʱôr{H?éH¡ß/È<?ʱôr{H?ç'‰mÙé?É$èUÅ?Ñ°í%æL-?É$èUÅ?Û§¤AÆÒj?¼©hÔ?â,-ß–Ë?¼©hÔ?èÌYá¸?®";YF?ÌÏú˜{Ñ!?®";YFMIXED3FGL J1512.3+6622@Yò¬![š[@F•ÿŽÀùÀ:ÏDÁ~À<,)d}XÀx½VQ@Œ©-oz@Ô UŠ÷¿ëÀK÷œ¦Œ¿ÔÖr@Aí¿æ»™i{¢@¿ÙL…Ç2UNASNone@™ê~($PowerLawnone?ïܹoÞñN?'k1$ðí?q£Hù$?'k1$ðí?ïá§eñ1Â?ƒ¿w¯N	?nXš,ÕÄ?ƒ¿w¯N	?ïÊ:1?™ðãZí\E?Ÿ¾æ°"È?™ðãZí\E?ïÿý®ÁôØ>°"㊊>²ˆ•Tò§ó>°"㊊?ï•èÖSðS?'æÄŗNf?Š…Ê]E{@?'æÄŗNf?ïC&Žñ0@?ªߤ"±?—›.j\?ªߤ"±?î>a®.?¢à
¤?û?¬î2‹*?¢à
¤?û?ïÿŸe"?ܧˆâ?&«
'x`?ܧˆâAGN3FGL J1512.8-5639@t‰ÞÒ?ðxÆj²üAÀ8«l)ôÆÀ:y*GÒ&©?q»I*ß@X"©Èeà@³J'Á¿ä7hˆ:ݳ¿èc#ÿõªM¿ç®Â¾+g¿âb¨ÄYážUNASNone@¥YJôðØPowerLawnone?ïæŒ~Õô?u+E~a÷?isÿFÄj?u+E~a÷?ïxkYÞ«?¨œ `?ò"Ó#b?¨œ `?ìáv‡Æ³X?©ö»Ó^?¸ôKÀ€ŠÀ?©ö»Ó^?ï÷¸s×ñ¢?7럺á¸û?P¨¼D?7럺á¸û?ï!ÓZGA?¡¨K~§§"?›Å­ò?¡¨K~§§"?ìSéÇÄ?Äçú×tz?½`´Ç!ß?Äçú×tz?ê批ý'=?±ŸñސTÞ?ÄeÙ	·?±ŸñސTÞ?ï¬Ð,£?t®ðӛ'Î?"Ëõ…DM?t®ðӛ'ÎAGN3FGL J1513.3-3719@t½Ï€Ü3r@1u)wȎzÀ:Ž»üÊÀ;¯=×Ñã?'{,¤ë@¨>?úõ¡à:õ¿ï£ŸB"¿?Ə`"¯ì?Ô?~~¶¿àMÔ)–UNASNone@ÀT§ï²-PowerLawnone?ïý¥‰ß3Ï?1Ï_%)?2Ó±Î}ùç?1Ï_%)?ïÇ&iÊ{?Ÿ´L¨V?|lË»bj?Ÿ´L¨V?ï՜fþfÎ?m­ª®xþ‹?u1̈[½?m­ª®xþ‹?ïì7íh^õ?Q¼ƒÛ?¡ï?cÈdÆÓ?Q¼ƒÛ?¡ï?ïøúœW¨Í?I¤à45B?LŽf‰â?I¤à45B?î—í·J{ò?¶îº-±ëª?¦$ëõä?¶îº-±ëª?ïÆ95^dB?{ñP³vb|?|ãe_<:î?{ñP³vb|?ï§ø-½lK?ƒ¸ga¤dî?†ô"‰?ƒ¸ga¤dîAGN3FGL J1513.8-6250c@sædobÀMݤõîÀ8SŠÁ'À:Ü»ÛãÁ?ÜA¿¼Ý°9@?' *læ@¨V¿ªOt¿Ôîà·ª¿é"K"W¼¿êª{GZBÓ¿ãìÕò]UNASNone@üµsê³hPowerLawnone%?ï⑾•Ó?rnð–à¢?mnA".|"?rnð–à¢?ï>Âè[m?¥£·z?˜'£.f?¥£·z?î'*î/ö?žkbú#²?­QÇŸ?žkbú#²?ïZ·-u¦m?w¦Ð¦Û}h?"©Vrœb?w¦Ð¦Û}h?íÈ+õ/+?²–e×ê?±¾ X2m§?²–e×ê?çÉïíZ®D?Çö7"ÁÄ?Ðl %J£x?Çö7"ÁÄ?éöM½øô?³š?'?È&É.?³š?'?èó²ÚˆL??³¿'äv?Ì14•ÞÏ?³¿'ävAGN3FGL J1517.0+2637@DD¾´ .@LÓ!ž¶9À:֖»˜ÇãÀ<®U¿ôŒ•YîÞÅ@
Åë Ík@ÄÕ"?ïÿ‡à'/ ¿ëÿe8Çz[?Éc G†¿äO€ڋkUNASNone@«zV»˜ÇãPowerLawnone?ïþèú?,@ (À©?!pQ€¾?,@ (À©?ïàöºOá?Š"©,Ä
/?o	ç
–Öù?Š"©,Ä
/?ï^T¿Ór·?'ãâ
ëÛ?"5h"
)?'ãâ
ëÛ?ïÿŒÎ ?wqߘwó?œÉ£U`?wqߘwó?ïþ
¿Ì‰0?2²!gqy?/Tµ${<?2²!gqy?ï['@"ªt? u>ÿá?"×ô's? u>ÿá?ïOüü"9O?ñß$Á?–`l	:'?ñß$Á?ïü"²¤$?BA‹O¸aY?;ÚkäŽîû?BA‹O¸aYAGN3FGL J1517.6-4442@t‡JB®Ñ9@%›î=_ÜßÀ9^dµ—&À;=_0Ϭ?ßÓ-‡ç@C÷¾½ë^@²m¹¿éBÚx1¿ä[/Õ@õпèhÁú®(ê¿íÿ:Ó*UNASNone@…ò2-VPowerLawnone?얞Ð:?—?¹f•†ˆœ|?»K	~.I?¹f•†ˆœ|?ï0
V^?¦³ÍĈ?þÆÔl'?¦³ÍĈ?ëþð¼Hί?©*³/¨ö?À=ÜÅF?©*³/¨ö?î2p^H?ˆWÌ ¨·²?¬Øú|?ˆWÌ ¨·²?å~ø[EöÚ?ÉÛL_‡­'?ÕItL?ÉÛL_‡­'?åÖM‡¥Ú?ϛ"¼à?ÕÈSdð´L?ϛ"¼à?äÌ\Eêß¡?¾êғ­"Ä?ÖgGt*@¾?¾êғ­"Ä?àЗß!î?³èBÖá›?Þ^ÐAü$?³èBÖá›AGN3FGL J1518.2-5232@tEš¿4@‡;…èíÀ8ÔÜޒÇîÀ;ëÚ¯
Ÿ?ôèøo"@ŠìËÅ»¶@îÿ´€¦¿Ý;|Râ¿áhʧ·?¿âōñÎB¿îìӍ†:íUNASNone@•œöz—PowerLawnone?ÊÊ6itÒ?ÆÙXߝ½s?éMr}å¢Ë?ÆÙXߝ½s?ØÊß²W«Ž?ÆÛúKN÷¤?㚐&Ô*9?ÆÛúKN÷¤?åâˆCcŠ?²"55«ƒ?Ô:ïy8êÇ?²"55«ƒ?㡟ޓYö?§`:§k T?ؼÀBÙL?§`:§k T?"hšÕ 0â?žñê²s­?ï\»)-Ã)?žñê²s­?²€_hž¹?·u=jîI?í¯ôЫî?·u=jîI?Ç0^yj;?²•NL¨Ë?ê3èa %q?²•NL¨Ë?ÇÕdpÅn?ª€sm?ê
¦ýãÎ¥?ª€smMIXED3FGL J1525.8-0834@v,)³ún@C%žYò»À:©Yš¦	À;²X'hLð?ªf€‰@À—µ=å?úM]ÞØh¿ïÿܬhÔ*?ïه2X&?ßÔUq{¿Û†fÍz­×UNASNone@Ã@½²-VPowerLawnone?ïÿkß2f@?,-†Î?"ì²ÍZ?,-†Î?ïÑë'´W"? üò%ï?w
l×öb? üò%ï?ïÔ¹'îƒ?r?vRÐ
?u£>§é:,?r?vRÐ
?ïù·'|>À?:ÇþC(Ôú?I!ºÖ"µì?:ÇþC(Ôú?ïþ"°(|K?*J¹ªj…å?'´ùz"J?*J¹ªj…å?ï[ûåzT?¯Æñ"úª?´€Š/íy?¯Æñ"úª?ïÇÄd?çï?~È_8¢na?|Íô©°t?~È_8¢na?ïñ_¤çf½?`†€ø¹ì?]@µéº¥ú?`†€ø¹ìAGN3FGL J1526.3-4505@t˜Éšé$ò@#Bö@c^À9•xgðª"À;FKMÜ?Ú…`I
]@¥Vôƒu@#—Á¼M¿é—Gý¿í[ÌçFB&¿ÐG#H•¬¿Çh(ˆ¤UNASNone@¼å`A‰PowerLawnone?ïýèÉ,¯6?DÅùP'<û?0¹µU»Á?DÅùP'<û?ï£ïZ… ?›ðXI"R?‡;"ãî?›ðXI"R?ïÁÝ8»ïk?{à½Õ™;?c¸ÊU?{à½Õ™;?ïö½½ÿï(?9ÿ5Öff<?R"ƒË研?9ÿ5Öff<?ïûP?C÷Ù¤'³?@Eßнw?C÷Ù¤'³?íˆR"•4?¿lµÂ¼u?³¿ånob?¿lµÂ¼u?ïÏîÚ­?–¡zøf?œÆ$¿ÊR?–¡zøf?ïÒ¢‡(þ§?j  "°¿?v®¼'Þm?j  "°¿AGN3FGL J1527.0-3804@t܃ä%¯@.¤ÎóÀ:š'Í¥:À;€¦'F•ç?¦oÑòlÎ@6žK…@¡í`@1ž¿ä†¢Æê¿ì'Vv{ª¿É€@›ëGP¿Þ°4|UNASNone@–üè§æ›PowerLawnone?ïþ۝u`?"mñú®?"F%£Õ·??"mñú®?ïÆNë,g?‰ãاØi?|Øõ¸ˆ?‰ãاØi?ïÖë±êH^?pSè5?tŠ'?pSè5?ïôwÇÈè"??fW#7zc?WpUrŒ0??fW#7zc?ïýP¶"i?7ýX÷Âëg?5zJ_+´Ä?7ýX÷Âëg?îžd$u]Ù?µù‹ÈÙ?¦½¹†	t?µù‹ÈÙ?ïq'±T¤?Œˆ ãLÜ?'ÍÉ×6ùŠ?Œˆ ãLÜ?ﱐF½1?vÒ0¿™9?ƒ¸ãQóº?vÒ0¿™9AGN3FGL J1528.1-2904@u9ßý`é@6m
$F0fÀ:ˆäö=öÀ;¡míCdÚ¿ë;
ª‡½@
–cî<D?û%÷@=ݱ¿ëΜ¡n¿ÝÑäy;Ö¿¬¬àÐ
?¿èº³Î,UNASNone@ÀÂwPowerLawnone?ïûsÚú$?DË|èA–?B0—¤`¬?DË|èA–?ïÑh%Ж?Œ'@ŽDä§?w{ËÎÛ$ë?Œ'@ŽDä§?ï«·ü†"ï?†7ç UÍ÷?…ì5´?†7ç UÍ÷?ïþÑ}ûGM??ßa™?"èîÏíC??ßa™?ïòáÙíi?]¼iÂWN)?Z=ʤ-N?]¼iÂWN)?ï'`Ÿ°"?°¨E]F?ž;òé%¥?°¨E]F?ï"!y類?¹Ú?Ž÷¡‡…¸?¹Ú?ïób²Ê¤?X'eµ»]?Y:š2)H¨?X'eµ»]AGN3FGL J1528.7-2247@u€Jßø"¼@;Evš'^À:™ï)îçÀ;šXKñp?èÁǒ-ù@
ێ	Ãx:@ðßëb¿Ùz£QJ¾¿â-J¹6Âà¿â™3ÅÕ6Ô¿ïÿÆ×âYUNASNone@–|BÞÑ·PowerLawnone?ï¥MÆ?ˆM¦CNî?†½þbLúz?ˆM¦CNî?íxœQnò?°fºvUi5?´;uLVr?°fºvUi5?ìDµç5·?¥f›^x'ß?½ß2PÆRF?¥f›^x'ß?꩖TÕ$?ŸÛšHÆk?ÅY¦¯¬«o?ŸÛšHÆk?î:³¥ßM?±¯1J>¬?¬^"ÇYÙ+?±¯1J>¬?ލÛÞá?Ñ<—%(·?à¹tt?Ñ<—%(·?薵£‡Ñh?±ùí0¡[Ð?Í¥)qàºb?±ùí0¡[Ð?ӚyBáüà?´«ØÁœÅ?æ2Ã^?´«ØÁœÅMIXED3FGL J1529.5+6733@Yß1)Ë«@EŽ'_ét£À:ÄŵV­À<3r"XÀ¿ëg¿p³@;P'¾N@å
ŸÁ%û¿ÔÌ!nî'ï¿çnéÍíî¿ây|ˆD¿àÕõÀêtUNASNone@˜9':)ÇzPowerLawnone?ïô"Æy&?pc	ín?VØr¡Íå?pc	ín?ïàeì¢?'ln¸]š?ošýV¶OÈ?'ln¸]š?îð4¡­K?›-hc®µ'? ü¾ITÇR?›-hc®µ'?ïÿ7›LÍ
?—Á$T??"£)¤U?—Á$T??ïñ®>¦•?egÔt¾ÈB?\£Í¹¬•'?egÔt¾ÈB?ï.Ñß'º¦?«¤2EiÄÿ?š%ÄPÝ3?«¤2EiÄÿ?î«nïˆ?ŸÈ¼k‹?¥Niw£~?ŸÈ¼k‹?ïò%LsS½?Wñcé7Ñ?[µgSõ?Wñcé7ÑAGN3FGL J1532.0-2618@ucblvK@8ºˆ&«À:#Š·~‡À;†@Ú»¢Ù¿Øp™Ã@ú¯Åüe@uí οௐæº9¿â(GŽMÏÛ¿àç¡Ú…È¿ã¥1 Ö²UNASNone@ jÀƒoPowerLawnone?ïþ´àê2†?"[£°Î»)?$±ð†ÿ™?"[£°Î»)?ïÎû!¹Ó?ŒÎ¦Qôû{?x'uñâƊ?ŒÎ¦Qôû{?ïÔO`nx?x rÿås?uØOÖ
ÇÝ?x rÿås?ïúËn?0x~;ô^?DÒDÜÚL?0x~;ô^?ïýÈ3F9±?1U\±Íü·?1¾eÄM.'?1U\±Íü·?îü/
&?°¶{+äB1? =_VmC?°¶{+äB1?ï…3ߣ?(\ZÈÒ?Ž»8öw³C?(\ZÈÒ?ï»ã-êÒz?tP|Ïq]_?4'ït?tP|Ïq]_AGN3FGL J1533.8-5231@td <K	ê@"]¶ŠÀ9m'Y4À;
Vìu߀?âÎApQ…@KšÌ>‡?ÿrû?{ëß?í•ï{«ûz¿Ù˜Ù]Ý^¿×(>;é©ì¿åŒ2 2²UNASNone@²'ÿ¾vÈ´PowerLawnone?ïñù»~÷?[
Ûk9I¤?\ˆ¸ÄÎ?[
Ûk9I¤?ï ¥n†gÛ?¯jŠœØfª?›ëR0êҞ?¯jŠœØfª?ï®ðr»«µ?€Õ5ÜBÒ?"Cã`3ZÄ?€Õ5ÜBÒ?ïg‡‰TZ©?sêu¾ê¢?"ÜSâÝ?sêu¾ê¢?ï"(Út3?ˆëˆyo?ŠõÉxâó]?ˆëˆyo?ê5Mó0—?È~sÅÁã?Ǔ*È3=£?È~sÅÁã?ï*aèœ.?"=T@Á]¥?š³ÝUtY?"=T@Á]¥?íyùSœø?˜•
Jùö?´05aՕÆ?˜•
JùöAGN3FGL J1538.4-4656@t¢þÅm\û@¢—žÖÜÀ8•;!>>)À;còPë?ìºO¡þÂé@Ë­MÖw›@˘¿Ô쬿èo‡]"V¿êúÌ5¼ê¿ê"Îà¿ïÿ¹€Œ#ÝUNASNone@txB0üøPowerLawnone?ï€[p¥?Ñ?'êQÙ@Âv?é#çÞš?'êQÙ@Âv?ê
¿k?ÁUuÙ²²?Ç×ýæU?ÁUuÙ²²?îdJ ô=?˜F>Ð5½?©»Uñ˜?˜F>Ð5½?é=Æßo^)?£E%â³V?Ëä'B‡[?£E%â³V?îÃY—²?³9§I?®"ÊjÐa
?³9§I?Ñö~°ùÌN?Ϗ
Š¾E²?çÀ§ƒÙ?Ϗ
Š¾E²?é·L¹ÛÈ,?´8芫?É"͐ßP?´8芫?Ì^—KFáw?¬ðM¦ï?èèZ-.G¢?¬ðM¦ïMIXED3FGL J1541.6+1414@7­ ÝD@H2`=WyÀ:eøg…JWÀ;¯ëí#"j¿ß±‰ñ—Å@
#Ïj¶Ø?ÿš¿5Š{¿ï §IŸ?íx‹dw£Ð¿ãW}vö¿ÞÈfžùœUNASNone@°Yí'hr°PowerLawnone?ïþˆ¥©®?!ݙë¯0ü?'~dqˆN?!ݙë¯0ü?ïÝìeªò?…².՚?q	Íú×?…².՚?ïÊñÿjÆ?wà?˜‹Å?z‡-Û.?wà?˜‹Å?ï÷ѯöË?B"Áåó:Á?P]Ìaó½?B"Áåó:Á?ïüL%aRD?9¥ä®sœ+?=žÔ`þ¿,?9¥ä®sœ+?ïá"†Ú?ªSÐ{qÕ?œÃßËÿˆ¼?ªSÐ{qÕ?!àr?"¹Ÿƒ?ˆ"¿°¨«?"¹Ÿƒ?ï…sŒ6&$?ˆœÖï à?Ž£ïÚü?ˆœÖï àAGN3FGL J1542.4-5911@t4ÿ'+¾ËÀ
-\Äüô³À94If{_À:蟔…]¢¿ë—7'js@2·7dE@Ðà©-`¿æq-ãÀã¿å¹û6(¿êdV#Ö§u¿è¶u>_PUNASNone@†\L˜_PowerLawnone?ïՏ:^åW?uKOã°Ò?u8b×lŒ;?uKOã°Ò?ï–þ…ñ4û?˜iæ†)?Š@^'q1:?˜iæ†)?îÿW}•W?"~Š;Ü
Ø? º"·"?"~Š;Ü
Ø?ïý´k''?#û£çˆµP?2\¥gç;Ï?#û£çˆµP?îõÐ\H?¦§†ŸÊhÍ? ¢þQ'	|?¦§†ŸÊhÍ?ìÌôîæ
w?Ã\kN5JÃ?¹˜XŠ‡bG?Ã\kN5JÃ?ëåˆe>É?®QË¢öÓ?ÀiÞkÛ²?®QË¢öÓ?ïÍF.<î?qcǙ"ã"?y\ÿú"â?qcǙ"ã"AGN3FGL J1544.1-2555@u‹ÁÝ!ê@6œŽ:!dÀ9/Ô!Tä^À;Y 8ð?õ'ÏÐã1é@qɎ~ÞW@Þ]@L÷*¿×Û«Ë(œ¿çêeÜJ:®¿å¸y™§¿ïÿ§¿!>UNASNone@ˆÛSž­Õ'PowerLawnone?á—êçâIX?Ï´œ},Y-?ÜÐ*0;mP?Ï´œ},Y-?Ϋÿ52or?ÈÌt)q?èU2³d$?ÈÌt)q?ç-òXÄߐ?±•r*î{?ѤNv@à?±•r*î{?Ø}€ˆ?mî?¨Ï9[ã`?ãÁ?»àI	?¨Ï9[ã`?˸lª‰?ÆÔv {|?éà;$Õ^?ÆÔv {|?²@W0?½J1ì%‡?í·ÿôþ€_?½J1ì%‡?Ü·~ÐYc?¶¯J'É'?á¤r@—ÓN?¶¯J'É'?«.bßï?ój<×M?îMÞDæ±?ój<×MMIXED3FGL J1544.6-1125@vC`¿]x@@~Àð¸À9iW²n}À;Jǘ°eŽ?õºçG!}@á—YÎR‰@M`@1ž^¿Ájàܷ"¿çà–>¿æ	`m?¿ïÿá&Ž4UNASNone@ˆ%Ov_ÙPowerLawnone?áýh:6?Îò(üÎr>?Ü/÷‹ß"?Îò(üÎr>?Êpü0VxÌ?ÊJ»ÔÆ°?écÀóêaÍ?ÊJ»ÔÆ°?äzAð:e,?²@3e¡ß?×|‹5©?²@3e¡ß?Ô,'Nï&?¨¹ô—Â3?åé¶ý؈m?¨¹ô—Â3?̇)Zþd†?˓x¤pQ?èÞ5©@fß?˓x¤pQ?³·aJ?ÁÒþÞî?í‰ÝàùÞ?ÁÒþÞî?Úã:†¦‰?¶'JD›?âŽbö¼¬¼?¶'JD›?¢þMË«]¾?†Ÿþ"nW9?îÐ#Ô?†Ÿþ"nW9MIXED3FGL J1545.0-6641@sîἩiÀ"Á'Ýãu†À:'Ns*šÀ;r3#Bû?Ñ…cñZå@ûÉTrH?ú¿æŸÜ©º¿ëÖ€BÓ¿å"x†/Ú¿ª5.é€k¿µ\]è­AÜUNASNone@Áp
=p£×PowerLawnone?ïþšFµ"?Aƒ?ܛ†¦?&[•?ù}›?Aƒ?ܛ†¦?ïœ-/Z?˜;xüëùc?ˆôœ8t)Œ?˜;xüëùc?ïè狦"$?mªL-"ê?gt;¡K×?mªL-"ê?ïý›OüÂ?ÇIAà?3%‰\ˆDV?ÇIAà?ïþ~ff?*viè»×?(šu??*viè»×?ìÚe'½´?ÂâZAƒÈ?¹,ÓjB^?ÂâZAƒÈ?ïä{"Ç;z?u«6B;?k"ÜÿÁ?u«6B;?ïöfZia?I|"ئ?S3ãthŽˆ?I|"ئAGN3FGL J1548.4+1455@9¡ë¦¬§"@G–a©É"À8õªõâoÌÀ;g8¿E%?Ü26Âù~ @Ø"´Šá›@å­_Ÿ!ï¿Î¾¬ÒË-T¿á™n·©á¿ãJŸfy¿ÝT{eY©UNASNone@˜*a|ÚQPowerLawnone?ïüU<-¾æ?6­",u!3?=Vßž?6­",u!3?ïÖÖð€õÎ?‡ÎX効?t"‡Ëã±&?‡ÎX効?ïÊߧšä?zxÍÑß??z, 5á?zxÍÑß??ïÉS?1#?a"vÑ£Ú?{V`Užv²?a"vÑ£Ú?ïùè¨U¹?JÔø#A?H_'a˜wî?JÔø#A?îájLÁ'?®˜U¢£øP?¡é^Σƒ×?®˜U¢£øP?ɟpÉ?‰)K3t?ˆÍ©QÙ£?‰)K3t?î7ÿöM'?ž/1ÚI‹?¬/þãYÞ?ž/1ÚI‹AGN3FGL J1549.4-4832@tªó¡LìB@ìúi¾
À8²³8§{À:ÑuúÔG¿é1©´€@~A…†g8@ïš@]".¿çòŒEYa¬¿íc\‰ÿÙÑ¿Ó«›q,Šo¿èp³hÅUNASNone@|sd£ƒ'gPowerLawnone?B–q?ÂJ!»€c?§¦‹Öž˜î?ÂJ!»€c?ï¢Ãˋ?•€:}oÏ?‡O
éåØ?•€:}oÏ?íÙ"Êf…?¢€Ç®³dÏ?±7c_ôýÛ?¢€Ç®³dÏ?ïó&~L"·?Q'Ú«7FØ?Y³ÁŒB?Q'Ú«7FØ?ï &Û®^o?¥JdÙ³Ö?›û$'j?¥JdÙ³Ö?íSÐÎnk?¿
A¯DH&?µayàs£?¿
A¯DH&?에ôj±¶?ª¡ë2Iœ?»Cx\ªrQ?ª¡ë2Iœ?ï7×]ێ˜?'øÒC—?™BÖ_
?'øÒC—AGN3FGL J1549.9-3044@ueâ'@·€@2$<µ¬À:f6ýÃÞÀ;"¹
Ó'Z?éÞ~š²Ý@€n1áÏh?÷¦¿òÉ·¿îm~ÂÂ?ï÷TYb`·?»áéû—÷"¿¡Å«%.ÏUNASNone@ÅՁ$ÝPowerLawnone?ïúÊ5¶Â?DÎDO‰?D×+!û(.?DÎDO‰?ï®nÿÖÔ&?–K'ïnFá?"d@o?–K'ïnFá?ÚßE?‡¦þ·?ˆ^ûP'f ?‡¦þ·?ïÆñ=fà+?c³"ë1"Í?|‡aZþFI?c³"ë1"Í?ïõºœ_?S¾FA˜Õ?TŠÇ¯W¢#?S¾FA˜Õ?í‹PŠÔQH?Â(åÎÍO?³¥{¨ŽÂ?Â(åÎÍO?ï‡ñPJ?Š½a`G\n?Ž¬¼O?Š½a`G\n?ïk{¥+ý?…¯q>¨ÿ‹?'†3u?…¯q>¨ÿ‹AGN3FGL J1550.4+6027@W^qŸŒ¨@F‹ÙÂ~•1À:TcûRÀ;ïèwM>w?¬cª²h@jùÀöªÂ?ýƒ˜ Õú?'Wÿɸëû¿¼!`DZÅ@¿Éb>ÛÕJ¿çW
×ÈÃUNASNone@®wŸU›=PowerLawnone?ïþuM¬R¦?(Šàb´)?(«"éÀ?(Šàb´)?ïØEŽ!â?…$†Búi?sÝ9ö¥?…$†Búi?ïÌC3 /O?|ðëÓԄ?yÞf
Œ@Ò?|ðëÓԄ?ïÙº;Ù'­?Y'"Ì…¿?s"âL¡¶?Y'"Ì…¿?ïøގVÿ?PZ¦H—?L…Ʀq6?PZ¦H—?îå·ëzs?¯ø'š:¤?¡¯"HXÎ?¯ø'š:¤?ïªggmLŠ?†—Å6³ùË?…f&(y"?†—Å6³ùË?ï¬0Ü'?'+Î8Rnò?êyëZTÖ?'+Î8RnòAGN3FGL J1553.1+5437@Ue3]$žE@G•¶Ü gÀ:&¤¯wÀ<y_gn¤¿åZ¢ÕF\Ê@˜•¸Ž|@
eÿ¹3=¿Þêø˝¿á÷d¾¤µ¿ä]ql¡5¿é©Ïzã1NUNASNone@".V¡aä÷PowerLawnone?ïʤȐ–Õ?²õÞeÿÍÑ?z­››‡Éx?²õÞeÿÍÑ?ï۔;ik1?"¢[¬pƒB?r5â3í‰?"¢[¬pƒB?&†7Î?ˆb7Ÿ×àÍ?6[px?ˆb7Ÿ×àÍ?ïû(bIÌ'?2ÁW(Ý®?C^v#d~?2ÁW(Ý®?ïÝÃðÊ?"n;ãT$z?qwð=ž~?"n;ãT$z?ïÜG5–?¯X4H¬Î?ŸwM?4?¯X4H¬Î?î-Iµç¿(?¡rP®²õ$?­+d ¨&†?¡rP®²õ$?ï¥d1òÓ?€^3@W?†¦Ü0¯d?€^3@WAGN3FGL J1553.3-0322c@vñýÞ½@BJ^Ý)5À9mlÓgñÀ;Q'TPº-ÀYsä©7@Zž¥òîJ@€p]¶¿é2ŒÚø¾¿ãå×;K줿ì2©J€q¿Ä?"úÐÐUNASNone@€~´9XbPowerLawnone!?ïîݟ>/w?k,¶Ì@D?a"`~x1'?k,¶Ì@D?ïÏ"`Ö?•Fû¶â?xnÏøœë?•Fû¶â?ïǕF?'âx6›¾$?œ
^ß?'âx6›¾$?ïÿÿí¿Y>sõ¤@Lî>b&ñ¹{$Ò>sõ¤@Lî?ïi•£sj¹?œDÊm¦?'ÍKŽ#Ø?œDÊm¦?î­ã–E"Í?¸ÔrýÉP?¥!Ɵó6)?¸ÔrýÉP?í1<b~FÏ?¦ÎIÍÊé?¶véè	?¦ÎIÍÊé?ïÿøm[ðc>ày—šð>ÎK|id>ày—šðAGN3FGL J1554.4-5315c@t"Ùè>B[?Ö-íCdٞÀ7Üݸ­[À9Øró<£?òí±ÔxèŸ@76³t @
 8ð?ÜÖF±rÜÊ¿ÞGh¤¯!k¿åZeCё¿è°Œ'ãRUNASNone@®]í\ú¬ÚPowerLawnone0?ÂtÉÚÃÊ4?Å	À
	å?ëb͉O
s?Å	À
	å?ãuћò?ÈyCøÂ
?Ùû\ÈÒ?ÈyCøÂ
?ד!M‹+Ë?·%Gñ²ê‹?ä6oY:j?·%Gñ²ê‹?æØ*‹fG?¨Vç²2Ë?ÒOѪé3q?¨Vç²2Ë?¦•Š‹Âø?­;j§M=I?W%?­;j§M=I?¾ò€rxÖ?¹LùŽ{ø,?ì!¯ñ°î?¹LùŽ{ø,?֕•÷[¨?ºRDgÛRï?äµ5{"R,?ºRDgÛRï?Ѻx˲ŠE?°•Ûã¯×?ç"Ú&ºÝ?°•Ûã¯×MIXED3FGL J1602.8-1924@vç#$È6@8Oh7÷¾À9Þ_>Sø¦À;eéÁЈ¿æcÊ«Æ~@l˜Œ´Y@€õs}¦¿ãþö,RÕ¿çIQÈt£k¿â6©µF¿äžÙ—UNASNone@–‰º^5?PowerLawnone?ïÿ4ot? Š¾Ãã?r‰bÞ? Š¾Ãã?ïÏùE.eø?ŒÀ÷òäeO?x]‰ÉD?ŒÀ÷òäeO?ïՍQÑr¾?oÚ77uG?u9W'ÄÁ?oÚ77uG?ïýNä{?%á]±k²S?7…ŽË@T¿?%á]±k²S?ïûþ"Q°ï?C àÐs9"?@w…1ßQ?C àÐs9"?ïq3k^À?°°
¶¶?Ÿ±Ù™s_ò?°°
¶¶?ïdð‡3‡ä?-ehåq´?"aï¯Ëƒ?-ehåq´?ïËNk"º?r	ÒÝúû?zXÊ0å?r	ÒÝúûAGN3FGL J1603.7-6011@tLƒùdÀùà`þG™À9è¹/a›À;k½"J¥@?ôèâ'Äb@hScTc/?ÿeþ>´Æœ¿äتÐgzÒ?äÖ©G¿Ø&ã&³ü¿ëMãÃçÔnUNASNone@©Ü›=ÈKPowerLawnone?Øk5×
ª?ÍÕà<Q{?ãÊqey+?ÍÕà<Q{?Ü[fµŽC?Ï'd¨¡s?áÒL¥8øß?Ï'd¨¡s?çøòńÚ?µÅðê­?ÑðtöL?µÅðê­?å BORE?±6h6&+?Ô¿{a[uÙ?±6h6&+?¾ÉÜ̳?À˜ô1"v6?ì&Ä}¦|Š?À˜ô1"v6?¼ñºå;%?ÁMƒ…Ið(?ìaÈ£X›^?ÁMƒ…Ið(?Ð֌yJ™¬?·E®'¶¡i?甹ÃZ³*?·E®'¶¡i?ÕFIÑìW"?½ŒÏudœ?å\Û	Ô7?½ŒÏudœMIXED3FGL J1611.9+1404@;ÈnÁ~ºñ@DфV!uÀ9ÞÊ#¥ ¶À;¨÷ÇLZL?â~M±A^£@5»Gdâ@­_á'¿ßTû‹bZy¿á˜'xñ‹ý¿æÐB=šÈÌ¿àÇB+@UNASNone@•íé*0U2PowerLawnone?ïû߆&¹í?Co-Œì®?@çi~2Ì?Co-Œì®?ïÃ[(½û?'VoÀ…«K?~Rk´»Ra?'VoÀ…«K?ïØP
´t?'›q;PÁ?ˆ‰ì?'›q;PÁ?ïŸúÉà3\?m8ö~:…?ˆM‹bÄý?m8ö~:…?ïàS ¢3?t¼ƒOgˆ±?oî¬yzÕ0?t¼ƒOgˆ±?î#M"%Ls?µz{	JQi?­Ë-áÔÆ?µz{	JQi?îÊÉM£?¥j¼¨»–1?®ÃTGÖ?¥j¼¨»–1?ìx_(É;·?ª™×ïéA?¼=¹¶"D?ª™×ïéAAGN3FGL J1613.4-4222@uû_ïJ@t‹e#pHÀ9p¦]¨À:óˆBY@ä¿ûÚOÊB®Ñ@cƒ•vI]@zs 
Ìã¿â,3_%ª¿í— m‰¿Ûš+ošl¨¿åÁü¸‰1UNASNone@"`ú¬ÙèPowerLawnone?ïùi?ORóï?i?I¾[×?ORóï?i?ï¸ê_Y׸?W"o¤OA?Åh(Ú&?W"o¤OA?ï"D†ë¹?""Qü®6?‹.øÓö=³?""Qü®6?ïÿéDÛ.î>ågŒ—–B>æ»GЄ>ågŒ—–B?ïêf؞‰?lºÉŠcï?e™'e•ø"?lºÉŠcï?î;ú»ƒµh?ºE0 Y;Û?¬@TFۄ?ºE0 Y;Û?îcâ´Pæ3? Ö
M§oô?©ÁÔºµÖ? Ö
M§oô?ïþDƒè'`?*ʒšß?+·ÅŠ0Hd?*ʒšßAGN3FGL J1615.6-4450@u*™0¾@?û¹IbÀ8Ó%žõùíÀ:³ËE
PK¿ì@†÷ð*å@Æ4/²u3@~ó€jÉx¿ë`ûZ©Äµ¿çÒí!mc¿ã"T
"¿äÝ
ë-¿UNASNone@‰
õ\)PowerLawnone?ïŸY£VÔ? 'OAŠ"©?ˆ>隙æõ? 'OAŠ"©?ïª\Ü­s?•¿ÂtÅ~ï?…{(ÁõkB?•¿ÂtÅ~ï?K¸?ŸXʸS+?¥"_錰"?ŸXʸS+?ïÿ@Hß0Á?ú
ÌV%?öág›¼?ú
ÌV%?ïÊ´¸À?…"ô" %?zô%Š2ÞL?…"ô" %?íܙW'Û?½W"×ÁP?±7k§¨?½W"×ÁP?íŽ._™?ª×wôÎá‰?·›Ž‹½p¶?ª×wôÎá‰?ïõ¼®'Åÿ?KðÒ&`?T†¢ª½þ?KðÒ&`AGN3FGL J1616.8-5343@t§—¢H"ÄÀ½Õü woÀ8ZÉX¤À:ªí"Ãq?äèKË@]ÄKžäÝ@=Žà-&Õ¿æÔ¾+Qðì¿ãy9Ó>­¿æI"܍¿ïÿÍݐ`ØUNASNone@†¥ €sWæPowerLawnone?çk(+‡3?ËÓº0@S?Ñ)¯¨ñóš?ËÓº0@S?ëàŠ¡Úï?ÀEa$tQ?À}Õx—ìE?ÀEa$tQ?æKœqÌ\?´¸Ü'†ßV?ÓÍhÇgG?´¸Ü'†ßV?ëq¯' Ì?¡N 4
ù?ÃÆ9A·|Ñ?¡N 4
ù?Ðî1y¨@.?Ì]<VP?çˆçC+ßé?Ì]<VP?Ó5#"nêÄ?Ìä2­Yóo?æennȊž?Ìä2­Yóo?Ù8ßR"ÿ.?½\wiîv?ãcV¶i?½\wiîv?Óg"êÌÎ6?³ŒuK`?æLnŠ™˜å?³ŒuK`MIXED3FGL J1616.8+5846@Va
xÀ@EX¤Ò²ÀÀ:1ùˆºWÀ;ÿ1æ,?Ï¥#\óÃS@ǐ:`˜@ʅ˿î'ßÞCå¿âÆm1ܛø¿ïü"±Òæ?ïژߛSUNASNone@qäd™ÍPowerLawnone?ïþoNÂZÙ?4Eäû¦;g?)¼ròô?4Eäû¦;g?ïÜ
º'?"—a­ÝZ?qõòìäGÒ?"—a­ÝZ?ïyr¬½/B?Š`Kpöö?Ñªjå²?Š`Kpöö?ïÿÏ-ô? Rv-Ù¿?&!‰½¸J? Rv-Ù¿?ïðu8ï¾G?h˜Cà¬á÷?_Žj»˜?h˜Cà¬á÷?ï_ÌÞp?­ü\ç\|?Ÿ4]`Z?­ü\ç\|?î_AÓƒ[?¡ÿ¥ø&I?ªç4L?¡ÿ¥ø&I?ïÝaÃ'K?·›ãõi?qO}6yž-?·›ãõiAGN3FGL J1618.8+5520@U:rŸYÌû@E¹¿ðEwÙÀ:·!†b…0À<(‰hÉíõ?Ûrv¥"ä±@n@'â@œ?ÿIw¿áðÁ?·¿ãô™'ì3ù¿ãQ厾I¿ïÿo•þÉ8UNASNone@'<j~ùÛPowerLawnone?ï øÑ¢{?·
£ðP-Â?›àåÞk°¨?·
£ðP-Â?ï7¤:B­5?¡Š+îiX?™xµò‹e?¡Š+îiX?ì«õÈ}?¬¹™[ýë?º§ Wù¼?¬¹™[ýë?í(HƒZ?—>˜¾"©?¶»¼S"ª?—>˜¾"©?ìÙqѲr?ÅՔÁ‰Ì?¹4qroDm?ÅՔÁ‰Ì?ç}Þ%?ÍØéþ-d_?ÑÁCÓá¶?ÍØéþ-d_?èq"'Oع?¿Ny	×W?Î;wbÀ?¿Ny	×W?Úl¼ÎŸW@?½xþ2dE?âÉ¡˜°T`?½xþ2dEMIXED3FGL J1619.0-5014c@tÒy»­À˜?Ÿ¶a-ºÀ7á€hp+âÀ9©{rg%©?ñÂC@–ÕU‡pø@s|‹5©¿à2׶=r¿é'¡˜Êr¿èíçؘ¿å²8]$ÚUNASNone@˜ÔkÓÃaPowerLawnone9?È4h£"©§?Êæ:­·?éòå×–?Êæ:­·?îZhΗõ?¸ï)Ò °?®JYuª5¥?¸ï)Ò °?×ï¼$wÈR?¶‡¹Ìv?ä!íÄ×?¶‡¹Ìv?íÞ¨ˆl?0ñOéf?±R¿{¼ ?0ñOéf?Ç,Aã‹fa?È]?/Y£¤?ê4ï‡&h?È]?/Y£¤?ÞéŠ5×?Í`§ñ˒?à‹:å?p"?Í`§ñ˒?Ù/«@'s…?¹Æ¯k+áÊ?ãh*_¾Æ>?¹Æ¯k+áÊ?å1q«e?¶n¼Sá\/?՝ÿÆ©6?¶n¼Sá\/MIXED3FGL J1619.1+7538@[EÐ|"µÝ@A¥ïÝëÙÀ:ԛÀ»F"À<%ZÞrç~?âÀùɞÞÂ@~¨Q˜?ûg€)†¿ïõÜíù›?îã†tù§ ¿à"m¾‰-?Âs¿Æ»!UNASNone@¹ý'A [ÀPowerLawnone?ïö"·» [? ŸÂ^ç?R֐Æ8jt? ŸÂ^ç?ïÙ䨜Ó?ƒV'Äœ å?sq
®qF"?ƒV'Äœ å?ﶲR3dÃ?ƒÿ{X5€%?'Sk€IK?ƒÿ{X5€%?ïðè!*áÅ?NÀÏٓ¤ù?^/½¬ü&q?NÀÏٓ¤ù?ï÷¢qëî?XZ§Ò՗ý?P»s²Ø?XZ§Ò՗ý?îçñ7Tö?¯rø&Ü?¡€ìŒv>¢?¯rø&Ü?ïcÞ¤e¥v?'Ès£p
?""+sKQ7?'Ès£p
?ï•óÉT·?…Ùg\R×?Šƒ
Ð?…Ùg\R×AGN3FGL J1620.0-5101@tËa\¦Ê¿ä?ØÝý ÓÀ7çÇj<"À9Éb¯ø€°?ñÖþí|l@_†`ÔV@[€YV³¿Ôꔉöt¢¿Ü{õv[žY¿çÎ3¹¸?n¿ãf1R2|ÕUNASNone@¨Ø^ߤ?æPowerLawnone?Å?;û¿åš?ƉêòÄ?ê°1š?ƉêòÄ?ë$´œÌ¡P?"žW¯?Ãm-ŒÍz¿?"žW¯?مî6?¶…8Búl?ã=t}ˆõe?¶…8Búl?ë(Ä0`¹?žã±Ù¿æ?Ã\ï?ú}?žã±Ù¿æ?±=QÀ`.ž?µzÐùfº?íØUÇæ;¼?µzÐùfº?ÎDb²Ÿ†?Äó×¼J°?ènçSX9?Äó×¼J°?Üó¨ð4í?¸j±NÂ?á†+‡å‰?¸j±NÂ?Ú§¯~T¼?¸7Ê̶_?â¬(@Õ¡÷?¸7Ê̶_MIXED3FGL J1620.8-5149@tø}¿H¿ô™@
6IhÀ9
Ñ­ÝÀ:oê3åàš?à¹+¤bd=@™Ä6%@»Õ@Ž»o¿ÞmW°¯Ï€¿í!]'澿CD?S)üT¿åµµAüàÍUNASNone@µ8>BZîPowerLawnone?ïÀú"ŽËh?ŒNÊxÊò?'µœm€)?ŒNÊxÊò?ïA3ӅèQ?°;
Q™y?—Ù…‹ÓYð?°;
Q™y?ìéÙÅٓ…?©"‰à,D?¸±1ÒJÙ?©"‰à,D?ïÕHrpÆù?a¬ªu»j8?u[ÆÞIï‡?a¬ªu»j8?îÀõu"ß?ª÷Ô®à¬?§#ðª_€?ª÷Ô®à¬?ê£ðKÆÁµ?É)S‡!Øÿ?Åp>Ðäù-?É)S‡!Øÿ?ì4*]1ðy?­¡Æ)?¾^­p|6?­¡Æ)?ïqVšýƒ	?Š®õß0K?'Õ,§.ÖÎ?Š®õß0KAGN3FGL J1624.2-3957@uQ¢3œ¿@–ž^$x…À9 €©ÌÀ:³À~à°¯¿ª´‹P‰@×´>ág9@(‰ðü¿ç"[À×1f¿äEmG¿æ?d€¿ïÿá{ýɼUNASNone@ŽlHK]ÌdPowerLawnone?׿L¾lV?ÔåOpç¯ã?ä Y ÉþU?ÔåOpç¯ã?ïQÛä[£"?¢SDHúÞ?•ÄƒrÓÁ?¢SDHúÞ?åÙÍ·aa?³‹&ŸKì?ÔLd'=ï>?³‹&ŸKì?îÞ¾Óԗ¶?‰Ææg%õ?¢¶"?‰Ææg%õ?Ó]ê	&Lù?ÐGû°ÿ«‹?æQ
ûlك?ÐGû°ÿ«‹?æØØD‹[z?ÏÉö+žqù?ÒNOvéI
?ÏÉö+žqù?áðÌö%Œ?¼]›&6 {?ÜgÊ´é?¼]›&6 {?â×T yÙ?½UÀÔ!?ÚüQW¿M?½UÀÔ!MIXED3FGL J1624.8-4233@u4®}Vlô@…`&±EÀ8ËAøÈÔÀ:¥Zs¿èʔŒ6@2ˆ9tëº@:×@H÷¿çD"8­¿èCÂöÆV¢¿æxþH𴳿楿l¼íUNASNone@†UÝcˆe•PowerLawnone	?ïŽàîöJþ?–gÝ^ëGâ?ŒGÄL¼p?–gÝ^ëGâ?ï¨ÀÑÙ?•ŽyÄ?…Ïà<;%¸?•ŽyÄ?툢<¸›?¥7(hÝl¶?³ºîG¨?¥7(hÝl¶?ïüœg÷'z?-Ï"J11?;Àzåì‡?-Ï"J11?ísEÞö3è?¶xjù1Õ?´eцA?¶xjù1Õ?íÉvIö?½˜òÊ^f?±·ÄN!kÎ?½˜òÊ^f?ꮧ'x	ž?±ØÀ×{?ÅEa¶ه?±ØÀ×{?ïÀ™à")?sül<1;9?³?ú?sül<1;9AGN3FGL J1625.2-2845@uØ_ôö@,fÃb(À9xx·¡ÂÀ:ê$=Ìê)¿òôv	³@ÁþÙºF@)¾×ü¿êÔ½âvá¿é¬ë';¯·¿á»<QÈ}:¿ÓBBÏ»óUNASNone@"C·škP±PowerLawnone?ïþŸÀ—Æ?*†¹íÔ»€?&¡ï‹hÞ?*†¹íÔ»€?ïËՋ.¿(?'úiê´§?z:jD4?'úiê´§?ï"]§ûÝ?‡mTŸ¿?Šè•ý™"š?‡mTŸ¿?ïÿâ<º_Q>âq7h˜µy>íÃHghµˆ>âq7h˜µy?ïýTÚÖXo?>0½ôKEä?5Y(õF…w?>0½ôKEä?îö@ž"6Ù?±³uŠ•? ›ö!L.k?±³uŠ•?¤-àþ? ù4>3?§µ¸Öm,? ù4>3?ïþAÈæýê?'ûûßí÷?+ão3fI?'ûûßí÷AGN3FGL J1625.6-2058@v:®záH@3I§;BÌ-À9EÓ)Þ À;"Pg÷`?ÓXŽ-ø@
g%Pq‡'@SÏÿ²'Z¿âž¥ñQø¿ìáWb+]¿âøLòì¿ç¿ˆOªUNASNone@"[–=Ć­PowerLawnone?ïý²tÿ'à?3SEvº'²?2lWˆO^Ö?3SEvº'²?ï ÇóõÏ?˜1ñh_æ?‡Î	ž%?˜1ñh_æ?ï"2È1æ
?…
3Kzà?ŽóN´‰y?…
3Kzà?ï6PpÓB?z 'qÄÍ?™5ñãäiÂ?z 'qÄÍ?ïööu"ýí?X=Áv–V?R–H6?X=Áv–V?êõà/ÑÕ?ƺ#ž?Ä(›@¸­?ƺ#ž?î_C`857?ž¼ÆýLi?ªÉø1)™?ž¼ÆýLi?çì´8¬Cë?²á¨•¥?Ð&—Ž§x*?²á¨•¥AGN3FGL J1626.2-4911@tër{²þÅ¿«Ýqà˜ÆÀ8|‡5DÀ9×ôm$Ɖ¿ðÞ	îkX@PæMÒEÞ@ÚÁ`ˆ¿ç%—=$¿é«´x÷¿âì7È]¿ß¡Ìts€'UNASNone@¹-PowerLawnone?åã®Ä+Ç?Ш·ƒ(WÒ?ÕÈ8¢w¨r?Ш·ƒ(WÒ?ï™A‰QÙ?š*Z?‰¯¹z9Ì?š*Z?㨋­{V?µ?À9Šs?Ùð®è¥	S?µ?À9Šs?ïÿ‰þφï?,srÿï?
€[zŞ?,srÿï?êÊދ??Å5k
©Àó?ÇÄԅӿ?Å5k
©Àó?ìþ<yj?ÃUÐ×snã?¸71?ÃUÐ×snã?è4ÆBü?³ˆÔƒp$?Ï,æ÷à¹?³ˆÔƒp$?ïøªJ¹.,?H¯öðšÀ?MVÕdefš?H¯öðšÀAGN3FGL J1626.2-2428c@vð†nD@0ä^	}À8Y
×ÊVÑÀ:]$
üB?õ¡¼Ö_@ÇWC]ͼ@3õ§:A?ïüçEا¿ç@Îk!P¿ã¬¡gT‰*¿çÒ^ö@ʲUNASNone@¡ÁþšPowerLawnone ?쓋]@ÍÑ?»<&óp
æ?»c¥ù'|?»<&óp
æ?Ù¡TË«±ì?Îe-ÃÔøã?ã/Uš*'
?Îe-ÃÔøã?çq¡Òðt¿?²"¼Yô?ѼZ'?²"¼Yô?áÚÀ$•-?³Ecŋàª?ÜJ¶Õ¥Ë?³Ecŋàª?ÝƵáμ'?οsh,*?ᥡ·?οsh,*?ÄõÕmü?Æõ°¾Ð?êÏŠ¤¼Á?Æõ°¾Ð?á՛IÎ?¶Ö¦L"}?ÜtÞÉÏld?¶Ö¦L"}?ÆjyXäü!?®b莫?êea©ÆÀø?®b莫MIXED3FGL J1627.8+3217@Jz©?)
»@EšÙ¾L×IÀ9ÆñÃ&ZÞÀ;ÐÈ1\™^?õc\†=Ç6@úË²@=?Ñ|4?ïߞÎ.C,¿àã­±K	¿âÎ"žv´N¿ì"äΏ£UNASNone@"w€4mÆPowerLawnone?͟±ƒãá?dzÒ\D¾?蘾_?dzÒ\D¾?È©6F|Ö?Ïâ!þW‰T?éÕ¹òn`Ë?Ïâ!þW‰T?ã§nû¥ß?´œ–~¿?ر"	È´B?´œ–~¿?ÍÆb1;??«Ý3x?èŽgs±0?«Ý3x?¡DÎÍ>Gõ?§Ä/³5œÑ?îë³,?§Ä/³5œÑ?¸söM_ë^?È`³\kïE?ìñ6Je?È`³\kïE?ÈÕàÅ.?³ÖqÞùüÚ?éʇø~δ?³ÖqÞùüÚ?¡*"kÏVÌ?‹½–¨‡?îí]ÙzS?‹½–¨‡MIXED3FGL J1628.1-3344@u£"úÖËS@$¼[òoÅÀ9ÉÔQüLÀ;7ò<ÈÞ?¼Ií´ÎÔ9@Ùéù-}è@îÉÿ½åÔ¿ëõŸûø"U¿ãg€¯è»k¿à)«[I8¿ÓÌȝ4¦UNASNone@©A¼j~úPowerLawnone?ïüóË`³k?Gõô&m?8a¢ï›?Gõô&m?ïâM´á?¡o_gÒHÎ?ˆ‡lˆxæÅ?¡o_gÒHÎ?ïȽĤ½Ã?vÍ믛i?{¡¶£?vÍ믛i?ïëú¤mÕh?KÂXfešÚ?d[Ž?KÂXfešÚ?ïódÇæð ?^JjÖ¼Q?Y6p¥`²?^JjÖ¼Q?í4ñÌ?ÀU¦§Áqò?¶Xq ]+u?ÀU¦§Áqò?ï{òŽl.?Œ(ɑ¼?œ¡¬z¬J?Œ(ɑ¼?ïå-ì¢U?æйScÎ?žcZ;Œ}d?æйScÎAGN3FGL J1628.1-5740@tŒŠ\å´$À"yÔØ4	À9²¥ùú,À;#áâއ	¿ÚS'nGË
@×qýÉD@¶ RÛÅ¿å@+=U¿éÐb×CPë¿èV™µ{Õí¿Ô۝Fï UNASNone@'ö–»˜ÈPowerLawnone?ïð­B¡n?lP໔²©?_Ä¥£øt?lP໔²©?ï"Fiysè?›œÌú'?‹.e¡£?›œÌú'?ïA¾YþŠE?4ä‰
!ª?—È4¾véY?4ä‰
!ª?ïúÒWù¸?3ft†æ_ý?D¶£e¶'?3ft†æ_ý?ï¢^MÏR?‹¼ÒN"?‡|hzJ›p?‹¼ÒN"?ì'+4r^¨?Ã8ejE¡¨?»v¦\m
½?Ã8ejE¡¨?튑¢eJ?¤…áŸÐf÷?³«ríAé-?¤…áŸÐf÷?ïþäÞ!Å?…ýl·?E?Œ€FÏVÆ´?…ýl·?EAGN3FGL J1628.1+0254@1¥‹'¡¡@@t<òϕÕÀ:L(Àª'À;´Ì3?æ"ßÉ\]'@M÷Y¾7@ú'ßk5¿º["'0®¿ ÷?$‰ö¿êP*v˜…¿×b2¢ó9UNASNone@5\wškQPowerLawnone?ïøäMG?X@›»s?O nfÕ°e?X@›»s?ï˜÷D'÷±?¤/ÆhÅìR?‰Â.Ô¢ÛÂ?¤/ÆhÅìR?ï=Ҋ•´w?Ê_;"5¢?˜E®¦j99?Ê_;"5¢?ï¥1Ýj R?qZä
"?†³ˆž˜³ ?qZä
"?ïÄ6€'?"9‡?äÄS?}÷dÙÔO?"9‡?äÄS?íP/âéG?ÀjUœ7¼?µ~€æÿ¯Ì?ÀjUœ7¼?í±­–Èü*?¥cÐ@ìü?²r"HÜ7°?¥cÐ@ìü?ìߓôiü?¯EÂ€N·?¹`\·"?¯EÂ€N·AGN3FGL J1628.2-2431c@v(C€ˆQ@0ƒ	"ãÿïÀ8wÒ<çèÀ:dVè'?âöZ'@H÷¿>Ä·@ú`Ãd¿çp^{¥+¸¿åM#"qÑ¿è@Û¾hl6¿âUQ©üúMUNASNone@™â,1&éPowerLawnone0?éûÅ7?ÑP¢?Èë#"Ç·?ÑP¢?îvÿ€©2¿?­¯Vòºy?¨õlÔ?­¯Vòºy?è†Z ñÞ?²²ßúÅ:?Íæ•|9Ȋ?²²ßúÅ:?ìA±™Ñ³ø?žY]'¢òm?½òs1r`<?žY]'¢òm?á	'ËÃYÔ?юJ˜L	?Ýí°hyLX?юJ˜L	?Þ *=§f?ÓcEÅ1"?à¯êá,L²?ÓcEÅ1"?␬ey+?»¡Å¯nw?ÚÞ§5
¨à?»¡Å¯nw?ÒõÕf›·Î?¹C™ÖiÿY?æ…L²$?¹C™ÖiÿYMIXED3FGL J1628.4-4546@uô!-w@kOÚ2æÝÀ8`É{ßtoÀ:aùӖª?ôxËéM!@ª˜zµ©@6 %#ü¿åî_ª¿é'*u°—¿ë9hÐ調îà#ñ÷©šUNASNone@"%Ðå`A‰PowerLawnone?Á5ÝBÌê?Á`¢wc¹¹?ë¹òˆ¯LÅ?Á`¢wc¹¹?Ì}ÏN1fT?Åè}ï2í?èàŒ,s¦k?Åè}ï2í?á—}fsû?·<´ù1ßÀ?ÜÑ3Ï	?·<´ù1ßÀ?ß
җù¾?¬·.õžÃž?àz–´t¡?¬·.õžÃž? q3•ûª?¦uÑ$‹ª¸?îøìÏ1è?¦uÑ$‹ª¸?Ÿ¸ú©Ï?±0ËG892?ï? Sòñ?±0ËG892?θMCª¤¯?½9Z ª;ö?èQì¯VÔ?½9Z ª;ö?³&­Å0ÝT?›)}D
?í›*Gžœ…?›)}D
MIXED3FGL J1628.7-8056@sm‡~äâmÀ5ŸVûW÷À9àÁ3;–¯À;'yLò÷Ú¿À¢XÕâ©@ÿ‡Š#@»ß"¥"¿àzò ­¿êððØg,+¿çúe:í<¿ïÿ€
HСUNASNone@{²¢H"ÄPowerLawnone?ï¢Éd&?–RR Ea1?‡{z†._?–RR Ea1?ï—ZÌË?"t[
ñ?Š)zB~d;?"t[
ñ?í¼C·²*×?ž¶µf?²âBµÅ?ž¶µf?ï-í%ݵ'?Ap^?šB[@Ù¿?Ap^?ïULÒZo?¤©hxBí?œuVgl€?¤©hxBí?év7c_Ì?ʌî¥å'P?Ê'!Âr€Ñ?ʌî¥å'P?ìR)A†¡ß?«´	Êh Q?½nµóÊñ?«´	Êh Q?äæ{øä?»œZ" 2û?×Ä3é9?»œZ" 2ûAGN3FGL J1630.2-1052@ ¹™aÝ@8È!~|À9ºV4¿û-À;Y¦ùÔlÔ?òz(»
-@7î-ð~@a« §U?ïRÇ:f®5¿åIøopƒÔ¿å!'óˆß¿ïý…¿û‹°UNASNone@ìs×ÛõPowerLawnone?Ú~¸ÿ@?јtμš?âÀ¹#€@`?јtμš?΄¦ÌÓò?Ò·Q¯Žè*?è^ÖyË?Ò·Q¯Žè*?ä°'˜÷?³ëý¸;Á?֟ÖúÎñ?³ëý¸;Á?Ó͐§,ª-?°g©·Lr?æ7¬iªé?°g©·Lr?¹HOIö5?Ác©ƒÙ?ìܖö?ü‰?Ác©ƒÙ?¸ºp+¯?ÊX[4H?ìè±úäb@?ÊX[4H?ҌNœ4y?¹2ÉQ;]®?æ¹Ø±åôD?¹2ÉQ;]®?¦÷1k±´?'J~ÐÖÌÊ?én)e?'J~ÐÖÌÊMIXED3FGL J1630.3-6126@tcGd­ÿ'À!Í_™Ã‹À8ÿXz™À;\l <K
?Í´#¼%hM@–)€Výh@I`p-:¿éÀGáɒ¿èTia¿æ¯tҏڿïÿϲUNASNone@vµ}ÔA5PowerLawnone?ïü;ú¤mÕ?DB›òaÄ}?> +ŒTƒ?DB›òaÄ}?ïrë¼Ékç?Šà8ý\?'¢ˆ_óK5?Šà8ý\?ïs¾Ç.?Ž©¢-ñ?œ1'ÿ°A?Ž©¢-ñ?OšÑ?mv@IT[o?ˆ`òøƒÕ?mv@IT[o?ïúŽX•9Û?R…Ë+n
"?EƝ©ÿÖ?R…Ë+n
"?êÐJ£<Z¤?Äo1?ľÕs•o?Äo1?î*›"*$þ?¡È:ಥ?­VFÎ9—"?¡È:ಥ?ì%Wþäµ?¦m"¥O­?¾ÕAâÚU?¦m"¥O­AGN3FGL J1630.3-4346@u2SâÖ@	†×:ÇÀ9ˆ³c$"À:ˆpSO?ðrD˶ø$@
mœ@Ô@P`j£ã¿ëA2'^>¥¿æùdÌÍ…¿ë|[Ñjžã¿ÜœJ°jUNASNone@·'ŠáG®PowerLawnone?ØHÙz?ӈ$öžF@?ãÛô"Bðô?ӈ$öžF@?îx®Æ}Ë?µ¢IuÒ°‹?¨uØ#U?µ¢IuÒ°‹?á3i§
 }?·ÕÇöí¶?ݙ,±ä¿?·ÕÇöí¶?îЫ³Äàg?'Ãf¸?¢õDčà"?'Ãf¸?Ц© U~?ËãJ{Â?笫/Õ@ö?ËãJ{Â?ߥ'}ƒŸ˜?Ó&ì¨à4?à-lA>04?Ó&ì¨à4?áÒ2¿ðÆQ?¶*…§®·?Ü[š€s^?¶*…§®·?æ€@¢\‹Ç?ëþ/49Ý?Òÿ~»Fèr?ëþ/49ÝMIXED3FGL J1632.8+3838@NÞáG®{@EldE#öÀ9àõø?A^À;áý¶z?ð[(ã#%t@.£yè@žXߕ&m¿ï̦¨1@?çJ<M§í^¿åvzÊeX¿ïÿ—Ö²UNASNone@žýó¶E¢PowerLawnone?àØPž‡§?Òü%Ĥy
?ÞO^ÃÀð²?Òü%Ĥy
?Ô±-¶ëN?ÒÌYN$ü?å§i$ÿ
Y?ÒÌYN$ü?æÈË1°ëß?±}´Þ.ú?Òniœž(A?±}´Þ.ú?Ø:{.'Ó?¶ï¼÷Çm?ãâÂsh¾—?¶ï¼÷Çm?Üd~ûï¶B?ӕMn»?áÍÀ'$ß?ӕMn»?Â-_Ö÷•p?˼ª9hÆ,?ët¨
B¤?˼ª9hÆ,?àdè"H?¹ÎÌVZTµ?ß6.ý»Ïq?¹ÎÌVZTµ?¯°ÙøÀÌ?¢É¹#H?îò`/?´?¢É¹#HMIXED3FGL J1635.3+4257@Pèñ€
|@E:ž¡@WÀ:O&ò³À;òøK֘(¿ò½Fâ½yô@-Yôèõ¢@U1\¼™¿êîÛü{Í¿àÏñ´&§x¿à$'rŒB!¿ïô'½ÌµUNASNone@Š4mÅÖPowerLawnone?ïÖÎ΄²Ø?sÎx|s-?t˜˜Ó¤
?sÎx|s-?ïÓת:?†?‹<V6\LK?v*æÿÅ?‹<V6\LK?î¸;9€Ãú?•šç_eº?¤|LgÙi?•šç_eº?ïþí|k¶?azÖBŠ?!/¥E?azÖBŠ?ïº g©‡x?u*>âÓ?wæÏíÿ?u*>âÓ?î¹!#¼Ñ?´xƚ–Š??¤míÅöé?´xƚ–Š??í›üG°?«(ˆ{¸RÚ?· Îÿ?«(ˆ{¸RÚ?ïëÓ¿Ÿ¦?aôaŒÈþ?d,@–™B/?aôaŒÈþAGN3FGL J1639.4-5146@tä
"M;À
ËšþôgÀ7ìú@£À:®ŽwýgŸ?ãÜzª@>`ÔV.
@ËBàO`¿àüöøoh¿äÏ>"¿äk°ã«á¿æÇ1'ý¦½UNASNone@'"dxGPowerLawnone?ï5н$ì§?¤8ë®	IG?™Eè`‰Õ?¤8ë®	IG?ýmÿb?±»i'b‹ß?¦¦à'h;ã?±»i'b‹ß?ìJÿ$¸Ç?ª&ãÊÄ?½¨Ú9ÇÍ?ª&ãÊÄ?î
⛄ð?ßŒÜؤ?¯QÖKü'È?ßŒÜؤ?ç|
mtÖ?ʟÍeN
?Ñë%SÃ?ʟÍeN
?áÝ`$5?Í¥X<Š¨n?ÜEñ?·"Æ?Í¥X<Š¨n?åýÿ?¹K[9ŠÛÔ?Ôú"'É?¹K[9ŠÛÔ?âÕæa¦ìœ?¶	oqPE?ÚT3<²&È?¶	oqPEAGN3FGL J1640.6-4917@uÕ<ÝÖà¿ýX™¤T(À8Y'£Ü»À:aÙïÊþ–?ìüÞ8¿_@A9ˆâ½$@tÿÑ¿äÞ~r
l¿ç~%q ù'¿ã0¥c@0¿é›XL-'DUNASNone@œFTɅðPowerLawnone?î͘ŸÒ |?¥ªÎ›|Ž?£&vM"6?¥ªÎ›|Ž?îÁ@•Ø€?´ê½ƒÆ®?£ëö¡œY?´ê½ƒÆ®?êÖ=†?Â?±6ŠžD@?ħ	ç÷ï?±6ŠžD@?î®kÔ 'í?€LEˆ2Y"?¥B¶ÒÈ6?€LEˆ2Y"?ç?-}oJ?ÊŸùì%ê?с¥!kÏ?ÊŸùì%ê?äû·Æo)?ÊӎE[1ˆ?Ö	Аs!­?ÊӎE[1ˆ?äZŸÞ#®¨?»ô´|¸b?×JÀC¸¢¯?»ô´|¸b?éÐ/$0?ªo ¯"ß?Ëà¿C³o??ªo ¯"ßAGN3FGL J1641.5-2856@uü«¾Ê«Š@&ÄÝÛ
À9™­»ŽÀ;6Õü÷7?먕_ùõ@tî¹[¬@] A"ô¿âH`q"Ó¿æ´æB®j%¿ëU¿]´¢E¿ÜhW΄C,UNASNone@"&Ì~($PowerLawnone?ï×óq|D?I«‹ÚÉ?tG.  ü?I«‹ÚÉ?îýC	Ñ ?©:]O	ª-? .ÛÏbíû?©:]O	ª-?ïTø–«?€#‰™‡«?žaìb›?€#‰™‡«?î}¼Øc?ŒÑòé{‹?¨/¤/
3Ô?ŒÑòé{‹?íè_•ä¦?³¦<Áܖµ?°½	™Õ?³¦<Áܖµ?⇬È(*õ?ÒCn)S`z?Úð¦o¯ª?ÒCn)S`z?ëA|]YÞ?¬	þ©ã?ÃòúŠ˜†?¬	þ©ã?â®f™"a?Â>^!?ã?Ú£2Í»<à?Â>^!?ãAGN3FGL J1642.4+8045@\oÁ½¥@?ÁP¹U÷ƒÀ:A)Ý:ÙÀ<u^Pî/?ÜíÔ¤v[@j×9bL@áz AÙ¿ÞÎÕù#ö¿åÐ×b¿é÷Ös¿åSCTF0ïUNASNone@†ÛF?PowerLawnone?ïýí^Æ<˜?6$ëÐ
e
?0•>ûÒ?6$ëÐ
e
?ïºR<Éñ?‡µœӛð?kpÊ!$?‡µœӛð?ït'»l
?‹_Åú?'{'~Oð?‹_Åú?î筍¹³ã?'+M)D?¡…' õ%Ù?'+M)D?ïë]eÙ/?mš''Év?d¢š6r?mš''Év?ëѺ"˜"?Á£›j ¨?À¹íŸw¡?Á£›j ¨?흦X'3?©­Fx?³Í<RN~?©­Fx?ãß*¢À߯?¼§ò¸CÓ¿?ØAªº~@£?¼§ò¸CÓ¿AGN3FGL J1644.4+2632@G;Ž!–R½@C@oiDg8À:*=h@[:À;¯³æKùÔ?Þr[…?x@
÷û%$ҝ@–ˆÌB¿èmsZ›Z¿î¡·ú~a?Ò½š¡Ä4¿ê,9ÓÐUNASNone@€wޓž®PowerLawnone?ïúª£'%µ?LÒ·olÛ?EUqœ³~?LÒ·olÛ?ïªå—|'?—¬—éz´?…Fš Û X?—¬—éz´?ïk"©® Î?ŠgŒ<k?'jÑ7?ŠgŒ<k?ï Ë&sK?yûéW‹o?‡ù
%5!S?yûéW‹o?ïô+
Iê…?cR£m-W?W©äó8·!?cR£m-W?퓁žiü¸?¼î¨)Tb-?³cóÕÛ¿?¼î¨)Tb-?îӌÿy¿¬?˜ž‡y]í?¢Ç0	?ì@?˜ž‡y]í?î»ÿ*©2?¦Y
";?¤N 1SÝ?¦Y
";AGN3FGL J1644.6-0911@!ZWɱh@6ßpyåŸ,À9¢{…²\À;5£"ŸY¿ÕÑÝHו@
5ré×u@‹³ŸÕý¿äÈ^gƒ5Ä¿ì{"'È¿Úqì"õÆ¿Ùp9Ðþ'UNASNone@‡\ƒa@OPowerLawnone?ïü*`.r?Cמk1E?<«ÖÇ®Ü?Cמk1E?7>
_?©+ƒ ÔŽ?r7[à?©+ƒ ÔŽ?ïw¨¿7Ÿ?'Õ}á½*?ˆ¢×P3?'Õ}á½*?ïû1§AøÉ?0ĂªÀ?C9bxû?0ĂªÀ?ï÷b×)‹Ù?Wåñ7Å|?Q:R#ܯ?Wåñ7Å|?íÒôýe?Á>ÌÓ÷?³'o—|-Ú?Á>ÌÓ÷?îâVþÈ?—ùôñ¾{?¡ÚžÌ¨G"?—ùôñ¾{?ïÐ6­ÕÕy?q§~X{d?wä©u?q§~X{dAGN3FGL J1646.9-1332@ÏV!tÄÎ@3ä_ö"FÀ9ý»´v"²À;R]¤öÄî¿ó²¼ökÕ@
äË+­-?ý›ÃNúº¿îå±ç‡ýÕ?ÜŸŽ%G7¿áJé&¿Õä£ÖçáYUNASNone@ºhٙ™™šPowerLawnone?ïýr22¾T?4Œ#$,´?4nm;¯½ú?4Œ#$,´?ï—Øáz{>?¨Á°Ñ#¯?Š	ǤÐ̏?¨Á°Ñ#¯?ï¼Cwn?ä%†ÖÄ?€ï9(«æ?ä%†ÖÄ?ïÿÀ?"z>ø¸'PH½H>ÿõYܾdu>ø¸'PH½H?ïøûhZv2?J"߯ôÁ?L]ߢ¯?J"߯ôÁ?íµ9Õtø?Áy-<??²S†3&<?Áy-<??ï'0½É4ù?‰sÀë7ß?‹³Ð|"µÝ?‰sÀë7ß?ïûð½Sg?@;"\Ë?@=`0?@;"\ËAGN3FGL J1648.0+4230@PÄ:}ªOÊ@D÷œ"/¥À:kªKÀ;òÛé B*¿Ô\È/%©Õ@|s(@»Ý@×mŠNοàC±‰`¢"¿éæï'7ñ¿âŠ
î¥H¿ïç»ÊŠÁÿUNASNone@‹"Gy¦µPowerLawnone?ïý_ÔsW?1I𦗄‰?7©Œ5u?1I𦗄‰?ïÌp€$?C'—¼£?yÇÀ>Ž!?C'—¼£?ïyQã}?~Ö˜'?Õߜ½xb?~Ö˜'?ïë-èñp›?OE_‡jú¨?dÒMÈ4‹?OE_‡jú¨?ïýð¢%?'?3ӛ]y¡t?0zíŽ[î¤?3ӛ]y¡t?îZoeq&'?¸@©¸Q"ç?ªY	¥}úî?¸@©¸Q"ç?ïJ±uΟ?'§'î?–©Ý%d?'§'î?îØ1ƒÊi4?–. ÿÈÛM?¢|çÄ5S¾?–. ÿÈÛMAGN3FGL J1648.6-5635@t·k¤"ÈŸÀùõß덂À9CCÁð`À:ýàl¼Á½?ôSÈ)$@
)œ–¤Ô@hž\‹¿ãžõ"YŸ¿î‡Ú%—¿äJÅk¿ÐŠÙD¶UNASNone@€÷"àÞÓPowerLawnone?ìz6k29I?»_#¢­¥¦?¼.L¦n5µ?»_#¢­¥¦?çË9õͪ¡?ϵè36?ÐiŒdª¾?ϵè36?ìÑu‡&á|?¤"ô}»£¢?¹tSÅ&?¤"ô}»£¢?ìFXcP?¤孃\?½Í<çÅ.?¤孃\?êAþõéѕ?ÃÈ[-Î~?Æø(X¹«?ÃÈ[-Î~?ÅWFk|Ù?Êßìœo«?ê¿ê.e Ê?Êßìœo«?ê¡¥ˆó?­¾æÅí?Åyk™ß˜4?­¾æÅí?ßV	iÜ?Å!hkµkî?àTûK2?Å!hkµkîMIXED3FGL J1649.6-3007@vð¹@"Šl~®[ÈÀ9
д¸ÙÑÀ;!Š{¥?òEaƒ¨–@¸¦Í^Ã@"É﷿ߟ-ý¿3¿äõ힇¿â˜µ˜þ"¿ïÿôo±œMUNASNone@¦Ö"uPowerLawnone?ç/‹ÔMä?Ñ1Yx[O?Ñ¡ðèWd7?Ñ1Yx[O?Þn÷¢rd?ʵ$f´'?àȄw.ÆÎ?ʵ$f´'?çàè¥ÆM­?°äþ,å=?Ð>.´sd§?°äþ,å=?äÄõ¨?©=\iÓÒ?×úwóà±?©=\iÓÒ?ÚaIAΒ±?ӈ±>üÀ?âÏ[_¶¨?ӈ±>üÀ?¾
¢!tç*?ÃßAÞ5™¯?ì>K»Ñc?ÃßAÞ5™¯?эù¦I«?¶Àª˄l?ç9s,Û*?¶Àª˄l?Ä*1ë?§Ì˜ÍÖ\ú?êõ{½:³…?§Ì˜ÍÖ\úMIXED3FGL J1650.0-4438c@uMIº^¿–ˆë¡y6ùÀ7P+ÃÓ)À:
™Îr¿:¿´ñ{Nr,W@Lóin¯@«"¬î‹¿åU5_™~Ó¿ç²¹'[ÿ¿å™»µÎ- ¿ë	—B¯0UNASNone@rR²-VPowerLawnone$?ÒßS>ý}?ÑÄòNwÃl?ætV`B?ÑÄòNwÃl?ïVdzÕ?­c¥ó³?•'	š©Y?­c¥ó³?Þ@Évè%?¸Ü➺?àßõ›D‹î?¸Ü➺?ï«ËìÔ?vWÖ °?…
ô|+Y?vWÖ °?ÖÆTv—?ÏAôRLÔ?äœÕÄÿ49?ÏAôRLÔ?껼=ÕÅç?ÆÆ8ÿ%­?Ũèc?ÆÆ8ÿ%­?ãÐfèÊã?·u"ï¥Y?Ùð_2.j:?·u"ï¥Y?ìÌ@o8?¬ªºM#K?¿yÿô†>?¬ªºM#KMIXED3FGL J1650.0+0356@5Û;BÌ-k@<®ð®SeÀ:)CæÝõÀ;•ÙÔóü¿ÕøD¸0@[ÛB±Ux@S€?ÖY¾¿é¹€á¿â6 $š‹~¿Ý["¾¿ÖLn£UNASNone@¡-úCþ]PowerLawnone?ïÿÓ'ˆ>ò&-"m—ú>öz^{å"†>ò&-"m—ú?ï¸[Zæø¿?•CçB¸Å?é)N€à?•CçB¸Å?ïì´fØë?kuHB@B?cK™@%
?kuHB@B?ïÿ…LÁµÔ>û½nÅ%¢?¬ÍK\ÄÓ>û½nÅ%¢?ïÿ®·õ
•?çê´ÞI'?Qñö8ö½?çê´ÞI'?îl™V†R?·ò÷kÍQ¯?©6j–¾÷6?·ò÷kÍQ¯?ïäÒ
î?rð%…3OË?k-òH€?rð%…3OË?ïü°p±Õ?4¦Pâiæ?:|zÒtÆ?4¦PâiæAGN3FGL J1651.5-4626@u9²þÅm]¿ö~'MKãÀ8ÿÔqܼÀ:2¯È¿ÿÛÂMíɝ@
dy¤†²Œ?þ¿+ie?ç"LšÀÇ¿ãi‹™Ì<¿àŒŒ¾¿Ä¿ãì·£2UNASNone@Æ.¸Që…PowerLawnone?çÏ?ÓÕ¤?ÍDÊtØÄþ?Ða€XU¸?ÍDÊtØÄþ?؆òÖ?œèìX-&?‰'‰ÞCJ`?œèìX-&?ç:æÙ€`?´%§AÖl¼?ъ2MÚÿ@?´%§AÖl¼?ïÿõ¶~ˆ>ߦ:ߜA¬>ԓqæ©Ná>ߦ:ߜA¬?è-W`±h?ÈÓMsÀ?ÏJ¢}:_Å?ÈÓMsÀ?í$óTÏ?sr,\?·Øg=Y…?sr,\?ꭕt¶?®ŒÒ(zt?ÅI«Î-'´?®ŒÒ(zt?ïÿOfºf?íQBfÙ?5/q°F?íQBfÙAGN3FGL J1652.2-4649@u5ö_Ø­¬¿ûàÛwŠ{À8¹°,À:=yaë­c?™g¾yNªÆ@ët±­·‰@»ÍŸ°‰ö¿êí\Ò
q¿æÝËu'[ë¿Ö‰óü3B¿ãክ~ºUNASNone@´|Éã½PowerLawnone?í9 U"ï?À'°0ßÆÐ?¶6ýR¶?À'°0ßÆÐ?ïtÑ×+S?©Ïè¼¼ì?'eÅMjK?©Ïè¼¼ì?éª'ä»?¶+Ôà¦?ˇåUôm?¶+Ôà¦?ïôÈ_»ã'?D")Tõì$?Vo@˜·"?D")Tõì$?ëE'ú¾Í†?ÃAØÐı©?Âé¸Éé?ÃAØÐı©?ìòÕÀf?ÅßÊáNý?¿ÀoqQüÍ?ÅßÊáNý?êê¬àY'¹?±¬PìCÅ?ÄUL~™õ?±¬PìCÅ?ïµÜÆ??s¤Myö?'ˆÎwÊt?s¤MyöAGN3FGL J1654.0-4617@u?ž£Y5ü¿ùҌDF€îÀ8Ձ×ÛôˆÀ:a6=©®»?íÖ¯Ÿ?uâ@[ã‹U38@Ÿø-y?åÅ°óADˆ¿è6
g¾øp?Öñ\Û¿âSY<÷UNASNone@¸$Ç+JPowerLawnone?ï+¾Š>ݶ?ž,@ûÅ£?šˆ.½K³.?ž,@ûÅ£?îŝ(DlÁ?µ×ƒZ¥?£¦-~Lèå?µ×ƒZ¥?ë{ˆsE`Ì?¯€Ø([Ïñ?ÂÞ2ê|Ð?¯€Ø([Ïñ?ïSc7ezŒ?'*}`_³?•"™|†?'*}`_³?íGڃ³m?·]Tº'½?µÁ+á¼¹?·]Tº'½?è<cN4t?ÌÇ©¾;Í?Ïs¾Ç.0?ÌÇ©¾;Í?ê| PÇ2?°¢
 ?ž~¼ã:?°¢
 ?Õ4G?˜±â0yT?¦©O/˜?˜±â0yTAGN3FGL J1655.1-4644@u<`ÔV.ÀO¼ä!}(À9GeÆ-vÀ:jÏЍK­¿ö'kØ@
«Ñ?þäw¡!MX?ïýt&Ù?¼ú]‹˜ÇY¿ìDñ/
¿Í)ȃðnUNASNone@Ƌ½Òñ©üPowerLawnone?î×&íL¥?±³0ÑPŒ'?¢''Ï	º?±³0ÑPŒ'?ï—wé¤&™?žS6	±—ƒ?Š"!Ë?žS6	±—ƒ?êºx$»?®ø*ê?ÅmåÌ?®ø*ê?ïÿÝ<Jwâ>îB¨*¯U›>ñaë Áýó>îB¨*¯U›?êM«{ç?Ňï3eC?Ç«–ÉRe?Ňï3eC?ìï™ù¡þ?÷ÏmC­Ý?¸‡ã0 ãŽ?÷ÏmC­Ý?éàÓ$³FG?°¨í0¸?È|³m2ææ?°¨í0¸?ïü±×Ü}ø?Bgâ6#+÷?:qB)q›ª?Bgâ6#+÷AGN3FGL J1655.5-4748@u/€IQƒÀ1Ÿ<pɗÀ9	ñ}†=œÀ:v¦ ™@¿÷ú­¥ë§@'6µð@ü½¿h¶"¿äBVãVž¿ë}»Áãe¿çìѓ'¿Ñfn`¨-ÓUNASNone@¥@2:)ÇzPowerLawnone?ïD)׃£Ó? XZ@/ž?—zÅô³? XZ@/ž?ï›t%ø§?™§Å]@?‰"þyñrC?™§Å]@?ì'4u}†?«Y±øæ$D?¿n\TÓ?«Y±øæ$D?ïÿð:1¡…>݀O"ƒ>ߋáé~£>݀O"ƒ?ë`f³ý?¿Æý¢O7?Â~e3"	À?¿Æý¢O7?í
`iÓþ?Âáõ±{S?·¬ü²I'?Âáõ±{S?éËCV':=?²ŠâÛ¤M?ÈÒò§c
?²ŠâÛ¤M?ïþZ$J"?-K£"h?*^,E':?-K£"hAGN3FGL J1655.7-4712@u7P›ùÆ*Àhñ[!ŽÆÀ8ìùTëàÀ:O7iù˜Þ?ã·Ñ$m@
ñk?¦@ൟ´Á?ïÿÂ8&ì¿êú(­Âý¿É
~XJ™×¿ècÃ`\UNASNone@¬hø†YJõPowerLawnone?é2M/É>?Î)ðoÐX¯?Ë6˛@Û	?Î)ðoÐX¯?î枠ûžÙ?²p-Ë8yÎ?¡–ïj+y?²p-Ë8yÎ?èXCZj&?µ²6?úcU?Ϧžò–Wg?µ²6?úcU?ï8Ÿréº?'¬ÀÐË?˜ì¿"ȵ?'¬ÀÐË?äfKŽsÌ?Òi'ÄȤþ?×ó3hãi?Òi'ÄȤþ?è_LyÊÇ?ʾ;Ò
›²?΂ϾÔã?ʾ;Ò
›²?èôö:Y?²ýTdÕCs?͈/"'š?²ýTdÕCs?ír¹ñ·é?£ádgc?´j7¼8?£ádgcAGN3FGL J1656.9-3919c@u›ñ©ûçm@«€>~ÀÐÀ8ÙZo¸ÀÀ9o+-«3ö?îuƒ2Wž«@
pµÕduö@ŸÁàŠ™Ì¿ìzÛd%¨¿ä>lbm¢¿â~­®Ñ¿é¶Z'àùUNASNone@¤™Ÿ¾wPowerLawnone)? q^&¬þ?®>¶4ŠN?îøêv›p?®>¶4ŠN?í(Z3?ºu攧Ÿõ?³ö¿£!è?ºu攧Ÿõ?܅é§+±?´
j»çu?á½,j'w?´
j»çu?í¢Ò*¸C?›ÛX:Z˜?²én«‡ÂQ?›ÛX:Z˜?µNµVÏÊ¢?¼@}‰êê?íV)UAƒŒ?¼@}‰êê?Ú¶«ïmÇÀ?Ñ×2ZVt?⤪I ?Ñ×2ZVt?Ú=Á?·äœi!©?âá¦ö,?·äœi!©?åV·Ëø€I?ÀW€]Ú?ÕRhÿo?ÀW€]ÚMIXED3FGL J1657.6-4653@u>tSŽóMÀÙï_žÌ	À9à>™˜ÃÀ:zBf¬ÝC?Ò©BeøyÆ@!ЂŽæ@i=@}H«¿íޛ›^?ïý°X瑎¿ã¯ÉÈ4¿à"‹Y"‰UNASNone@¹]āoiPowerLawnone?ïË'©šÌ'?†mðJ4¿k?zl+0Š(d?†mðJ4¿k?ïb®ŽB?©5¡)®û?"ª=ÏÆÆ?©5¡)®û?íeQALa¿?¥ÐB­a"?´Õuõ.þŒ?¥ÐB­a"?ïÕ²%L?aÖ¶´ CÌ?u&ñß~K?aÖ¶´ CÌ?ïO[æcT?Ÿ°þfØ:?œ"ëcp?Ÿ°þfØ:?ë[¨\Õîß?Ç»Aé/?'^Œ¨D'?Ç»Aé/?ìâË׬¶?§ü´¶Ÿqœ?¸é§ïØÔ?§ü´¶Ÿqœ?îå¬øy¬?•_RaPò?¡®….À—;?•_RaPòAGN3FGL J1659.0-0142@1¥Åo@7èSŸºEÀ9E¦N³Â:À;9ÏÆl`?ç2ˆ?¡x@$'RxGå@Ž™`cÂó¿Ùœ{©Í!¿ä𫲱ÿ¨¿Úþ£ûXŒš¿ëÃy¸sUNASNone@›Éò-VPowerLawnone?ï¶y£ë'?‡^µ7ÇÒ?'a—-ÞQ†?‡^µ7ÇÒ?ïbÅr'?ªš"
/)?§Q¾
Â?ªš"
/)?íœç.'?¦e©q
×?·ûÆ$°ò?¦e©q
×?óº?…''sï-M?§—w$yZ?…''sï-M?î@áéáÓ?¯.vhè;?®Ûñãõ—Î?¯.vhè;?êO?Œ÷Ž†?ÇgtšþëÐ?ÆÃÌ!Åç?ÇgtšþëÐ?谅5€â¶?³#W²«?Í=ë)üu(?³#W²«?èÖÃ̍?²Õ#¹øÈ?̧ïÌðÍÍ?²Õ#¹øÈAGN3FGL J1700.4-4019c@u•ê~ùÛ#?ó/ˆƒÇ À82NÛËÀ8—"€ãÀ?òw"pèu@Ò]×K«Ð@'¯ŸëBY¿áÔ.LæÚâ¿Ü|ùÁm¿ëå¥:%"Ž¿å&"g3HŠUNASNone@'£n.²PowerLawnone$?¦¿Mëíº³?·œ+Ν®è?î"!
*•?·œ+Ν®è?î3…±ß°?¸P'=ՄŸ?¬Ç¤èÙÓ?¸P'=ՄŸ?Øî, icé?´3¸à5ÿ#?ãˆé¯ËN?´3¸à5ÿ#?îeX01ß?˜*Qڊœô?©ª|ø›?˜*Qڊœô?z¤Š./?¨Áç³±\?ïÄ*Íð?¨Áç³±\?áçë˄g?Ò–®á2?Ü0(h÷1È?Ò–®á2?Ú¼4m^Áñ?¶—¹Á=ˆ³?â¡åÉPŸ?¶—¹Á=ˆ³?èµÑ}zn?¿¶ìCh=?Í+¸º
H?¿¶ìCh=MIXED3FGL J1701.1-4930@u# ¥&•–À42ðîÀ9peÓÀ:«Wãä?퇩Þúæ@'$«@'ÛŸx€Å?¿hf±9ôC¿ì+4>ԅ¿èóO™'¿ÌŒ–"w8UNASNone@˜ý|"µÝPowerLawnone?ëYuoÌI?Äý
]ûM?Κ*@ÎÛ?Äý
]ûM?îÿú‡×5˜?­Ð…}¨®R? W€Ô؈?­Ð…}¨®R?êJØJIV?´îz¨þØ?ÆԞ׊ک?´îz¨þØ?ïdŽ¹R?~çºn+?"}Ž(Õ¿Ã?~çºn+?ä¿÷A?Њiƒ|)?×ҁÊ}ù?Њiƒ|)?å4|ëWÀ?ÍÏ)«ch?՗)ÃP€?ÍÏ)«ch?âÞÄÀ}¢Ý?Á:?ÚBvºF?Á:?ë'@ÜWô?¶íiÛ?ÃcþüŽ 0?¶íiÛAGN3FGL J1701.3-5216@ublvKÀüÂ]ÞÀ9‹i"ÙHÜÀ:öÔ2ò›"¿æzB÷ÔëÞ@4Èaƒ(@Ó«@`m¿á|_)¹À¿é|Ρ}¢¿ë—¨ÁæÐë¿Ïß:sCoUNASNone@""ÝÌcñAPowerLawnone?ïæÁJ–/?x0êCÊ?iç>ÌÇ)?x0êCÊ?Çcp?˜tFßôƒ?‰Pþ–¿ð?˜tFßôƒ?ÿ…K?šñ¼Ôâc?¥vî°ã'U?šñ¼Ôâc?ïþï@.>?É»¹?‹÷?!ú~ûr?É»¹?‹÷?î¡ô‹ÏùÊ?°«M$Æ ?¥à·>´àa?°«M$Æ ?ìðÝ
jTe?Âöí®Tø¼?¸y–e*Ô?Âöí®Tø¼?êß[W"'r?¶®ìÕmZ?Ò¡­º8?¶®ìÕmZ?ïäô)ÌY?h6Èš"z?kÖ¾¹FÝ?h6Èš"zAGN3FGL J1701.4-4654@uD¶°_¯À÷d»k{yÀ8M·Ñ"+À9ò™°?ÎL?ñˎ6.í@Žà®.@àyQû¿ßwB(æË¿ê¾þ¬Ý‡õ¿æ¢	sWvÆ¿ì¯2ՀiUNASNone@"48†YJõPowerLawnone?˜u"GÑÆt?­hõ4¹?ï<VíøkŒ?­hõ4¹?ä¸\ç¦[¹?ÉÄ8d܊?֏F0³H?ÉÄ8d܊?ÙþSÀÏò?´ÕÈ…?ã Ö˜?´ÕÈ…?ç흵»–Í?§™Ü1/')?Ð$ĔˆÒf?§™Ü1/')?˜Î–lÍ?¡†v$•"Ì?ï9‹L­`T?¡†v$•"Ì?¼vy%}4?¿âùb­?ìq0ÛPYp?¿âùb­?Јú'	&'?»¨òÎ¥PB?绂¾ûl·?»¨òÎ¥PB?Ñ-§†Iä-?³ÈÁ³¶?çi,<Û
é?³ÈÁ³¶MIXED3FGL J1702.0-5414@tçõ£KÜÀ"VÿÁßÀ9°—  À;-X'ßB?í,ýÜÂÂ@𽢍^@ càz(»¿Û}ƣפܿéʓõÉMð¿ë]b¢E¿æÑÑ䎵eUNASNone@ŠÝ}!ÿ.IPowerLawnone?ï'^f©¸?•­Ð	!¤±?‹¨f"ô?•­Ð	!¤±?íJp½
´?¸Ä'ÁøÎ×?µ¬zeÞ?¸Ä'ÁøÎ×?îU7dÄÆ?œlG8.ã?ª¬‰»t¦?œlG8.ã?ìé‰3DûÞ?–ä4Ã7?
?¸³¶d S?–ä4Ã7?
?ë8o>–£?ä9j?ÃC§ùs?ä9j?ӡъægA?͍Àµð	?æ/:ŒÌ_?͍Àµð	?è9E³Æl?¹¹"c°K?Ïë©0æR?¹¹"c°K?ÛӒn'Á?¼¾;$c#?â6Ⱦö ?¼¾;$c#MIXED3FGL J1702.1-2524@vWñ6;%@#÷Úè'®À:>4ð¢"ëÀ;_$Ÿòy/À
tq£~@	ºˆ\Zsê?ü&C@qŠ1¿ï§Í:Ÿ§ê?äiáp¦cà¿æaW1rÇ?ÈÕ%‹Õ·UNASNone@Âu`A‰7PowerLawnone?ïüE7ã?RdGKÇÀP?=ÖAÇA³?RdGKÇÀP?ïÆLﶠ?‹W"ÒÀ?|و3A?‹W"ÒÀ?ïeå8Ã.Ø?‰aTNxîZ?"CXâr»?‰aTNxîZ?ïÿÿæÄ^ƒ>]Zz>i{ø¢Fs>]Zz?ïﯞFZ5?dÇւ~(?`PazlûO?dÇւ~(?î¶ýifÆ?´ã̉—)8?¤)h»¥?´ã̉—)8?î·h£œ@­?™¬–ˆ~O?¤‰uÂÌY:?™¬–ˆ~O?ïÿõÍ»Îç>晘%'ó>Ôdp`/‰>晘%'óAGN3FGL J1702.1-4623@uLw[0À,Ò@ª;À8™Éõ÷¼À: 2:ð?ÑOš+(¼|@Xî>Œ'°@Cà) ã¿êÀ`*76"¿çèáçwY¿éG»¼•XS¿éÀNº«À–UNASNone@Z-ÅÖ8†PowerLawnone?ÐꩾÍ'2?хïâÀBê?犫 ™lg?хïâÀBê?ïm‰^Qß?£¦®©@î—?']®Ûü ?£¦®©@î—?á]ٙ'ȋ?·`ma®ûé?ÝDLÍ°në?·`ma®ûé?ïÆÜL5|}?c©²µ¯,Þ?|'ÙÚCX?c©²µ¯,Þ?ÑێTÃÃ?Ìüw•ìø?ç8Õðž?Ìüw•ìø?êÄY´?ÆSÃ(«'?Äóå.?ÆSÃ(«'?ã@Õܽ?·=w˜½?Ù~äUÄF…?·=w˜½?í­·6ž³Æ?ž;î"}(?²'FLÂ/Î?ž;î"}(MIXED3FGL J1703.6-2850@v.¿œb¡¶@™?¯BxKÀ9Úæùž¼ïÀ;1ç£è§õ?ÔîÒ¦U"²@
T£ºM@ЕÀœï¿è¬RV9¬¿ß‹^žµ§¿Ýhm¼	õ¼¿è1[âÔËõUNASNone@¢*—>«6zPowerLawnone?ïÀê>ÞÉ5?¯*~ދ?Šà~
³?¯*~ދ?îí~úÔ?¨ãAÄ ¢Z?¡/¾èR¼?¨ãAÄ ¢Z?ïŽNõ†a?‡¾dekzÞ?ŒlB¡·ñ?‡¾dekzÞ?î[0%?]A?‹=´×z?ªLý¯yÇñ?‹=´×z?靖	œ?Ðc½ç+?…Øý'ù'±?Ðc½ç+?â9·Íhl?Ñò¥hH­ˆ?یdÅ/'?Ñò¥hH­ˆ?îl§ü'i?ž)ˆÚÌü?§	5€6én?ž)ˆÚÌü?Ⓗ³eƒÏ?»dÍÉ´?Úڄ™4øc?»dÍÉ´AGN3FGL J1703.9-4843@u1³:}ªÀ¾ «†+À8ÀUM9n·À:¦ƒɕá?ôƒŒçÚoM@
ÉfÅ=@àVŸsù!¿æð¼ÍóŠÉ¿á€Knµ·ª¿ëMkÙ xd¿ïðÊã
]UNASNone@õØ­«ŸPowerLawnone?†j©3n4?«'áÎR?ï¦U[@o?«'áÎR?ºå¦·£?ÃUHP@?ì£]‹)?ÃUHP@?ÝøP–ò?´7<âß]É?á×´÷÷?´7<âß]É?Ó<
m·ú"?¨zE°'>w?æaùI$¶?¨zE°'>w?P>'~ÃR?Xâ»(æû?ï÷྾Ž"?Xâ»(æû?•]Õܝû?±ÌÌM«A}?ïUQ-'€?±ÌÌM«A}?¾…¸2®Jx?©õ‹¢~þ4?ì/Hùª6±?©õ‹¢~þ4?øã{ñÛ?†ú#НD}?ï8ºå!?†ú#НD}PSR3FGL J1704.1+1234@@;‡½Ï@=l§qÉpøÀ9d¼¯HWˆÀ;|ƒ-±¿ç¬LT'£@Í,݃©B@ªŠÿwïÑ¿çÌBºÔk–¿è᫦·d[¿ã5àçX`·¿âùs–G!UNASNone@"c²-VPowerLawnone?ïþ)	Iæå?-v¨S6?-om‰†c?-v¨S6?ï»ìùÄR?•íEo;—?þ1Ë­?•íEo;—?ïȬr1?x¿,6z÷~?{õwIcOs?x¿,6z÷~?ïý&…zÔ?(Núƒ"?7ÖÊ Ld%?(Núƒ"?ïû7°_G¨?IG:ú=Ü?C!?
«ˆù?IG:ú=Ü?î"~¶'Š?³àâ­ò‡–?¦¸–×a?³àâ­ò‡–?ïqòêS×?‹7¹Zßë?'Á½Eé?‹7¹Zßë?ïÊôb'ò6?sߜÝÉ^?z…ÎÍ4Q?sߜÝÉ^AGN3FGL J1704.4-0528@-Óp&É@4̽±¦×À9Q!Ð4`ZÀ;1°(QWá¿ðG˜7™ÊA@
ÖHtÄù@zZ Šy–¿·pCR…Ëì¿êW1zKuŸ¿ËdöU¼¿åù…µê¶UNASNone@Ÿ©^ž	PowerLawnone?ï÷(Ì$†?Z¦È†`°?Q¯Ðoöf?Z¦È†`°?ïšyž°€?¥&øöÎr?‰a˜a»OÛ?¥&øöÎr?ïwЩvË?‹I‹tE€?'ÿsh,?‹I‹tE€?ïþÉ*š¢?¢vE?#mW[Jƒ?¢vE?ï땐ܗ×?iY†	B?djnë'?iY†	B?íáÎã8°1?¿5"h§U¼?°ñˆäð£ú?¿5"h§U¼?îæýÓ³yr?˜ÎïÀ+yŒ?¡"Â4³à?˜ÎïÀ+yŒ?ïó¹¡)Žw?Uò|ÓEýÝ?XŒ½²bqD?Uò|ÓEýÝAGN3FGL J1705.5+0948@=ÃRü&V¬@;ó~€8Ÿ"À9¤œ«fKÀ;v¬Ö(–?⠝^då@žæ$a´@sï< ¿äËߏG0@¿ëº'fZ¹¿éØ/_Ìî¿ïþ±Ü[‹UNASNone@x¥§æšÔPowerLawnone?ïÚåkv'ü?pŠé>¦»Œ?rJ6ø5?pŠé>¦»Œ?îAÝ¢—?±Ý/«]I.?«ï'(j«?±Ý/«]I.?îýrè»ü×?Œr9`? (ÑsdK?Œr9`?ì–wû†•þ?˜˜L
Ç8¡?»L@#ËP?˜˜L
Ç8¡?ïD~ªTý³?˜q:]|}?—p*±ð­œ?˜q:]|}?ãGçæÓÅ?Ðó¢>ƒÉN?Ùp03úXv?Ðó¢>ƒÉN?í–ô¼2?¢þýÍOók?³H_£Ö=Í?¢þýÍOók?×uõ¹ï¿/?µYf&§>?äE# i?µYf&§>MIXED3FGL J1705.5-4128c@uÕϪ͟¿Ñük`v7jÀ8A[ñ˜^0À9?m?ﲕ:õ@{õ¬"óí@#9ßÊ«_¿çrèf›‰¿êãýVb¿àÙ¯Ü|S¿çÖ·p³áUNASNone@€«Ø§Å¬PowerLawnone)?Âá'Ö;i?ÆÇnyˆ?ëG¶
q%»?ÆÇnyˆ?í׳jÑ??ºëB²ñÉ?±Bd«Ÿ…?ºëB²ñÉ?ÞO a^êœ?´.2¿n5*?àØ/ÏPŠ²?´.2¿n5*?îG:¶#+î?–´Zp¸?«ŒTž©(!?–´Zp¸?ÖQ…ÖeŸ9?Νbpk+?ä×=Í0d?Νbpk+?ß[Á$"?Ñ斋áäÑ?àR~í¾?Ñ斋áäÑ?àÒËmt?µôÞøiä?ÞZiËÿ%?µôÞøiä?éBzð¥Þ»?¹›'ŸN†Ã?Êö=h…?¹›'ŸN†ÃMIXED3FGL J1707.8+5626@U-þ®û+@B@­ÿ'+¿À:THùn‡À<«ƒ¦é
?ÐA(J29t@
±[UçH@
¨_°Ù¿íÞ¸1+¾l¿Ô}À³l‡¿åY
^¨Ä¿êJØ3ÙµUNASNone@}D=F²lPowerLawnone?§¹ß?¢48ۂ‹û?ŽÞ–
\?¢48ۂ‹û?ï¿Éë,E?¦ÞÊ5¤ÄÉ?è¿*Ûr?¦ÞÊ5¤ÄÉ?î‰El#?žËv¶jµ«?®ï÷l…$È?žËv¶jµ«?í–׆ô?˜ñmÔkh?·IG÷¯\?˜ñmÔkh?îsid{2Y?«9Ш›âl?¨Éi¹(Áo?«9Ш›âl?åLI™þ.?ÐÅPʦ_ƒ?ÕglÍÖ¥?ÐÅPʦ_ƒ?ë[¦yoŸ?¯÷§Df²?'fŠA"?¯÷§Df²?֍äàûê?º¸tïã?ä¹
'
ÿ?º¸tïãMIXED3FGL J1709.4-0917@(d ]Øù+@1¹‹Å›€$À9ZtŠìW­À;"Øzøß?òŸDFx@L'Ûç@·Ðß´0¿à°2x*è¿ää0ÌÚj¿ï¡a+5…??ÜH¿,âGoUNASNone@†êæšÔ,=PowerLawnone?ïM(ìw%ë? æPl?–ZârÓœ? æPl?îçc~ªñ?µZëý°?¡‰Èǜî?µZëý°?íE¶;¡ýÒ?¢à?ñ1°ý?µÒN"'í?¢à?ñ1°ý?ïT¡íÐþ?"0pG%,"?ˆª×$m?"0pG%,"?ìÁ&€È<o?¾Í§¬ñ~ø?¹öËù¾†?¾Í§¬ñ~ø?çÞéš›?ÑÏÊ%±"?ÐB-çÄÊË?ÑÏÊ%±"?è<8ÕUÿ³?²'k1"åá?Ϫ¨3?²'k1"åá?êëJ•
ÏÎ?Å),`Óv×?ÄRÕ«ÔÀÈ?Å),`Óv×AGN3FGL J1709.5-0335@1Uœàuöý@4²‰üm¤HÀ9\åüH»[À;*½é§Ï¿Ùijû@&ë$üŽ±@Âb€}¾È¿ç;£g ¿éT_0o½¿à§mƒÕÑÈ¿ïýåғqsUNASNone@'ÿýVlôPowerLawnone?ïí¹6B`?an~"0¤?bFÉ¥<pb?an~"0¤?J¤`i?¤ÕNWz0?‹ÖmVçå¤?¤ÕNWz0?î›z¹×'?•®BŽ"¸?¦H_Îؗ?•®BŽ"¸?ïéÔµ`í?S®¤Ö×J?f+ìwùêõ?S®¤Ö×J?ïâÿ~¥ÍZ?vP6HÆSE?m€®F;?vP6HÆSE?ítiÊÛM?ÀJM…]¼8?´\±©'M™?ÀJM…]¼8?íß{ÑÃ?¤ÑÓHœ8÷?³¿ûè?¤ÑÓHœ8÷?îðsq"`?"Ô;æfû? øÈò*\þ?"Ô;æfûAGN3FGL J1709.9+4624@R÷´·@B1C¿rq7À:\ìOIoÀ;ðö'9)í¿ñ>ÜÔ׳0@
öÑÁŸ}@í ,ì¿äì>
ì[ø¿éÊñ"žÞ¿ÜI˜Ol¤Ä¿èA»püUNASNone@‡:·`¿]yPowerLawnone?ïÿ<Xeš? 
xBîʖ?tþZƒ¾? 
xBîʖ?ïØÄìûä?ˆ0啘f?sû}#v8?ˆ0啘f?ïÐßâº[?w¼Éi&õa?wœ£(×?w¼Éi&õa?ïþÌ)ÊåÓ?›¯(KCC?#=f"~?›¯(KCC?ïþñ.£Mð?$zP­Ri? í?­\±?$zP­Ri?îö"Ûïvè?¯{ØËuÄ? Ò?PÃ?¯{ØËuÄ?à%€S?ŠðXã³þ?ŽWHî¿?ŠðXã³þ?ïêdY¾.Ç?b!ÞR­`D?e›¦ƒÉ¸ð?b!ÞR­`DAGN3FGL J1710.6-4317@u'•éᰊÀãâ;ëiÀ8£bþÒÙVÀ:3T9¿ç+"Ÿ¸I@i›Â"¸Ú@6¤€}há?ïÞIρÝæ¿ê×{»Ñ싿奡mV"¿ç"§4•fUNASNone@'ó»~ÿ—PowerLawnone?çcÝo²?ƒ?ÐÒý';?Ñ8E ›€ú?ÐÒý';?ïŽj‰F÷? ¬‹‡Ö)?Œ~¥S_n=? ¬‹‡Ö)?æàv_$J/?··ÞsÖK?Ò?A·k£?··ÞsÖK?ïüµ+V¬?/F¼4…F¤?:V¤¨þZ¦?/F¼4…F¤?æJ@Ô µ?ά1B»?Ók~Vz¾–?ά1B»?ì¨[V›uÅ?ď'k¢ó?º½%K$QÕ?ď'k¢ó?ç˜Bø´By?´;ùY·p3?ÐÏz—{?´;ùY·p3?ïÝL=|?g?Ò$Þ(?qsYü¼!Û?g?Ò$Þ(AGN3FGL J1714.6-3327@v	9-Œ*@Q]À¥wÀ8ãÀÏhˆ€À:u¡¥×•~?èXç³ê@Ú_c<æ:@ۙ wï¦?ïû7»'U¿é¤f"a¿Î'èÉ
S¿íyü‰ÐyUNASNone@ ïƒ{J#PowerLawnone?ë´RÛLË?À{©y`"?Á/¦´'ÌÔ?À{©y`"?îòÉ-'x?²«Ãë¤>¾?¨ÓlQ¡ƒ?²«Ãë¤>¾?ä¬wùûrì?´º{]æ²s?Ö§	'?´º{]æ²s?îƒĀðM?ôFU¨<Å?§Ï3µ]F7?ôFU¨<Å?çŸfÝ(~?Ë5¹|©?ÐÁ3ôE¯?Ë5¹|©?ç"4lVë?ËSÆf+X?ÐٗÁ'R)?ËSÆf+X?äÎåt}D?µs7ǹßØ?ÖcÜ5x?µs7ǹßØ?댪]|?±»@U­?ÁÍW®Š?±»@U­AGN3FGL J1715.4-4028@u¯vݬîá¿òÇAÝðáÀ8çw ÈÍdÀ:qΣf¡ö?Ô©{¨±©@^9ókÇú@ÕYŸ®†'¿ïٙ{‰Ã?äæBÙ泿¯ƒû¿û¿á°ŽJ'ÛUNASNone@¯_oÒ PowerLawnone?ïæ)÷dë?hàó?,-?iÖ¦êÕi?hàó?,-?ïbæ!»O?¬¦~Ðݬ?"£;Ìr$?¬¦~Ðݬ?í§œ¨(
÷?¥@E'¯•?²Ã¿-ƒÅ?¥@E'¯•?ïé/ø|d;?Râý¼
Ë?fй5¬ç?Râý¼
Ë?ïrŸ
¦?'8PÍy¥?'¬S¦À?'8PÍy¥?ë¹;XÄ?ÇP'USÍ?ÁŽŸŒð?ÇP'USÍ?îàvçÉ?£Hd-2/?®ñø"÷p?£Hd-2/?ï¾,~–¼x?v¼
êpà?€tàaˆî?v¼
êpàAGN3FGL J1717.6-4404@u"^Ñ·ÀÌ2ùQÀ8nzj)i†À:n½º
Ri?ájÜÄÞä@›N•dUÀ@s¿ÀIÝ¿å \ÂVYÜ¿èl¬yxÅl¿ëºˆ×çC¿ãšá?S0UNASNone@…€¡ÿ.HéPowerLawnone?îòŸ`5?§†Ç©L? ×托¯?§†Ç©L?ïm!QŁ?®ÌÈRç?ž[ÒW³î?®ÌÈRç?éc›2 ç?³sçK†Ä³?Êq"5|c©?³sçK†Ä³?ïDxªâ?€âؼ(?¿×wÉÛÄ?€âؼ(?âG[ï??Ï"u~˜?ÛqH!Úá?Ï"u~˜?äWuù	j?ÍÉތNÄ?×Q
íÃ+?ÍÉތNÄ?â¢5
½?¿:¹a|¿?Ú»•ê"åû?¿:¹a|¿?ærªí w?¸kŠ{d<z?Óþª%¿?¸kŠ{d<zAGN3FGL J1719.2-2433?ß&•á(N~@E#ŸAyGÀ9Øïþ¯À:ëьO.;¿ê{—Ùƒ@
ti?´¡@QÓøÿ¿é®z'/Î,¿ëlîïr¥J¿Ó‰Û
àÆÝ¿éu;ss•#UNASNone@<NÄÑ¢PowerLawnone	?ï†QA1›?¤ø$¨ ³
?Žkº%dÅP?¤ø$¨ ³
?ïoTcÚoù?­Cvn¾›ÿ?'s†iÎì?­Cvn¾›ÿ?íÛã¼0%?£v=öý?± âÇ	_?£v=öý?ïû›ÊÔؓ?84wWö?AÓԏà¬?84wWö?ï_ç(®0?¢³ðئ¼ñ?"Zê9ù?¢³ðئ¼ñ?í#²o±ò4?ÄG»³þR?¶âlƒLUb?ÄG»³þR?ìž2å§Üu?¨$EvÛ[?»hÒÁY?¨$EvÛ[?ïÏa×áRì?rÛ½–$i?xO:"?rÛ½–$iAGN3FGL J1720.3-0428@1þ}ÔA5@1ìaAcwŸÀ9àÎÏÜKÆÀ;1s?'½À6·$ÄÛ@á=1¹¶p@°§ÀMãc¿åq3†6²¼¿ëØq›Dœ¿ÝèL@[ ÷¿Ï0Ÿ\H¢©UNASNone@±Ú>vÈ´9PowerLawnone?ïþ«@­f¢?>s0M1?%K÷c!âÙ?>s0M1?ï©j…ëøó?›"ȸÞ0â?…¥^P—'?›"ȸÞ0â?ï›ÃRÙr?Œî êÃC;?‰+P—›]?Œî êÃC;?ïÿÿä,§>uÛ<t7>k×.²5Ja>uÛ<t7?ïþ8§]É×?7­á~"ÔÛ?,uˆ%6*¦?7­á~"ÔÛ?îùXˆ?¼Ø"!H‹E?¯pj~×?¼Ø"!H‹E?ïN2±"H]?—¸pöH'?–9©ÐæW?—¸pöH'?ïÿýV,‡r>Âxï%P»C>µMùÁg>Âxï%P»CAGN3FGL J1720.7+0711@<ÿAJM+,@7i㸡œÀ96BhZ\mÀ;MbXº¬9?Þ9ëÜåý(@IŽ"«@Ï€oÑõ¿ãý>QŽ,¿ãgnöÐ"å¿æV	–¤=¿çãr3WŠUNASNone@'ŽÚ6âëPowerLawnone?ïÔ1¥¿l½?‡¸Ù³Œ <?uç-0Õt?‡¸Ù³Œ <?ï$å+\?§§ÙÐb®?›c_¿»é¼?§§ÙÐb®?ï4¡UXT³?n"ÈCJ?™kÕXeŽ?n"ÈCJ?ît6+=Îö?‰1ähDÃò?¨¼L#ž?‰1ähDÃò?íe9$õ$?µ8¶£H?´Ö7ß´=Ü?µ8¶£H?ézDÇ'?Ɍ¸Uä¨?Ëò–ìãe?Ɍ¸Uä¨?êO'Ì?³"
eŸò?ÅÂÃçÿ`Ñ?³"
eŸò?ãL0qP¾ù?¸¿7ì^?ÙgŸ^'?¸¿7ì^AGN3FGL J1721.4-5253@u·AJM+À"4!ž¶9
À9Dð(§üÀ;@Ø7d¿ÎÓ鿪X@
&<(zGš@­¿cØ¿ëÈÌ@ϗǿÞdÖB[3¿éó]†T(²¿éêF~OÍYUNASNone@‰m}ÔA5PowerLawnone?í­Kì×H?¸yOæáå§?·•¡u,¾?¸yOæáå§?ï~ån.\?p°[ê?<CWaž}?p°[ê?ìû0'e¾?£¬Š;q‰õ?¸&~Äi"?£¬Š;q‰õ?ï·nc¨?kõjl5?'$اP?kõjl5?àÆ#øt­?Î~N'ªÚ+?Þs¹Ä§?Î~N'ªÚ+?êGªA:;?ÅðÖJ´i?ÇÒáVû?ÅðÖJ´i?æ•Ï!]?C?µràí é?ÒÔa½E{?µràí é?êo£yA_q?²5'0…Œ?ÆArú'=?²5'0…ŒAGN3FGL J1721.8-3919@uÉÑc4'¿¿øs
=³À8·5@L À:B·
èa¿þŸ>+´¹±@A
•iß@Xwœ'"¿í±6i|#¿ÒSüÖC²Ì¿áã6+h¿íbZidz¢UNASNone@™ŠQë…¸PowerLawnone?²¾MñwŠ?Áí ñ–u?í¨6A§â?Áí ñ–u?Ò­?š7†Ó9¦?ˆ"KjÑH÷?š7†Ó9¦?à6á²Z??´¢*EŸW?ߒ<›ÅK'?´¢*EŸW?ïÿÌÂœb?^—&Q͖>ùžîò0o»?^—&Q͖?µBµ5&?»þ5Ô¼õ?íW©_½ÞP?»þ5Ô¼õ?í%Œôð'_?–#|u¶)?¶Ó˜VV+Ž?–#|u¶)?áފ̈?·+ªÝ‰"†?ÝèCÎêfï?·+ªÝ‰"†?ïûÓQm¨?DL¾¹u»?C€²Ìúqÿ?DL¾¹u»MIXED3FGL J1722.7-0415@2~µ^ñýß@1"BÇû¬´À9‡YûôÙÀ:æ+Íä$?ôëG©·ÉÛ@7´»³õ»@[ü€¿?ïûǪ+À¬¿àñ†»»¿ènÂ+øÆ¿ïÿ›ÞIàUNASNone@˜Õ;dZPowerLawnone?´NhŸ/g?»-Ò¡"$?ív2þUc?»-Ò¡"$?º­Ï[_¢?Ç@©N©—z?ìªFŒT?Ç@©N©—z?ÙS߸¸?³$è‹9òz?ãzV}#¤?³$è‹9òz?ËWpZÂ)—?¨ß{}´<±?é*#éOuš?¨ß{}´<±?‹âÆ·ž?§$Í]Ï´?tòßö?§$Í]Ï´?¦GÚc}Æ?½ÖZ»É€x?ZæÃ?½ÖZ»É€x?³—
m>?¤tAŸ¡_P?퍞^€?¤tAŸ¡_P?¾%jÔL?ˆM}Bh2Ù?ïÔóэ?ˆM}Bh2ÙPSR3FGL J1723.6-3646@uîΤ¨ÁU¿Øsš×\HÀ8›EÏíé}À9¢P¢¯ÂÑ?æ%c¤·@
Áñ§w¨®@Ìh€Z?žŒä¹ÚU¿è,E·3!¿ä*ï-†P¿Û£±[¾RóUNASNone@§n`PowerLawnone?ÚI˜Õ"?҆…º-|ª?âü[~3•6?҆…º-|ª?ï
èöEŽw?´¤»ÉŠÇ?žBá2&Ç)?´¤»ÉŠÇ?àýGùé»p?µ£¯Ñw(?Þp,‰ ?µ£¯Ñw(?ï‹ùÖEF†?tFä9Ö³|?Šu–n?tFä9Ö³|?Ó+
ܕ?ÍåË/'"]?æjzuùµ?ÍåË/'"]?çûM@^¯?ˎ[ôƒ±6?Ð	dåB£?ˎ[ôƒ±6?â»b°é?¹aÉ\ã'\?Ûډ:ž-õ?¹aÉ\ã'\?í-eü‰(?¤ÃŽ‡ø?¶"ÐÚØÆ?¤ÃŽ‡øMIXED3FGL J1725.0-0513@1ìh¹ý½0@0&cAøÀ9´â:¸cÀ;ÙÁfg¿ô¸Î¾¡@Û\ÁL$@%ÄÀcÝ˿ǃõ…0"¿é1̋‰`'¿àz»÷¬8¿Îxí|›UNASNone@°³S÷ÎÙPowerLawnone?ïû›9Vã¼?JÉjù¤?A"fcc?JÉjù¤?ï"tM®Ö?£%ôÊ+'œ?Šâì¿s'`?£%ôÊ+'œ?ï«Z¾´Ó~?€'ˆý@è;?…)PV:¼m?€'ˆý@è;?ïÿÙL>ëñý»ŠØ^>óZï—Î(>ëñý»ŠØ^?ïð\v?e¿È1¦xø?_Gi3ü?e¿È1¦xø?í¸Ÿ+~ß?Àµž–P?²?ˤ		?Àµž–P?ï:û‹sˆ…?'ÞÊÿÐ±?˜ ŽŠ¯·a?'ÞÊÿÐ±?ïý^Éu:¦?7#"õ…?5	¶aˆè?7#"õ…AGN3FGL J1725.7-3555c@uý—ÿCB¿ÏBwß4®]À8+Þº5"À9O·Xâ?Ýd"¼Ð@dZ­ Œ¨@Àè€1"¡¿ì·ºýþ";¿ãP¨¸V¯J¿ß‰DL`*ã¿ëw­þwâUNASNone@¨0^ƒä%¯PowerLawnone0?ý ¶ig?ÇýhFÌ~Z?ë—û'e¦?ÇýhFÌ~Z?ï7×üÅ|»?°‰Ã*'?™gPh›?°‰Ã*'?ÜZ÷xfL?²v›<ÜÕ.?á҄7ÃÌÚ?²v›<ÜÕ.?Æ|jy?|ÇÉWÍFo?Î]uÅã?|ÇÉWÍFo?Åo¢Jÿ=ô?Å쬾0õ
?ê¤m@0ƒ?Å쬾0õ
?émôʱk?ɒsÍ#¬$?ÊH,Ôõ:T?ɒsÍ#¬$?ácn©£Ih?µ´,¿ÕJ?Ý9"¬¹m0?µ´,¿ÕJ?íbP½»??¤S‹D`'?´ízÜ)?¤S‹D`'MIXED3FGL J1726.6-3530c@vÑ·Xâ¿Æ'ÍúI\ÀÀ7£-0º²ïÀ9‹Àނ÷?òÄïc$½z@eÛ­m0@u¹_݋6?ìဌò/¿æÐZ\± ¿æRT­p)ø¿ê΍Ÿ:mdUNASNone@ûÑë…¸PowerLawnone$?¡ŠÂó!xµ?²?þXòË?îçSÑâ4?²?þXòË?ç&2bd	{?ȧpÉä?ѳ›;7í
?ȧpÉä?Ïþ¦Æu<:?³ ÑÜ>o?èVNb°ò?³ ÑÜ>o?éì½#{?«Áӌ"þx?˸Or?«Áӌ"þx?¦Àøb²´?²§{E@ˆ?î"ðyòµ?²§{E@ˆ?ѯ»")?É;Ò¸êS?ç("w½ëw?É;Ò¸êS?Æ$m†|m?¹@&œpg?êvúäž`å?¹@&œpg?Ú¾)é)ò?¹¬CÈà6À?â ëkù?¹¬CÈà6ÀMIXED3FGL J1727.4+0634@=6cÇOµ@5¥yžQ?À9‰/Þê܂À;:³In?ï.ú81¤@W]"Dù@&À36c¿èEw¿çx¡È£X›¿êÝ\îSÁY¿ïùAû«UNASNone@'ŸêçÕfÏPowerLawnone?îE¦FŽ:?ªh—'«=ü?«¥› þêa?ªh—'«=ü?ãºh_ÿ‰?Í*.Sò½Å?Ùò‹/@î?Í*.Sò½Å?퇘|Qùâ? Ò;lTÌg?³Ã<'þñ? Ò;lTÌg?å¸OŒÛB?«xÛ=2?ԏ`æIË{?«xÛ=2?é™7»qõU?ٌeuòî?ɛ!8*®?ٌeuòî?Æ¿&_Ôì?ËVêê¼n?êOP6h
Å?ËVêê¼n?èoÙµF&?¶&²~9cE?Ïê@™*çh?¶&²~9cE?ÁØ9tbIï?¤‡@†äz?ë‰ñ¢çm"?¤‡@†äzMIXED3FGL J1727.6-0654@0Á‰&"Ï@.AðÃLÀ9A 6×,¢À;>Ä`î?âÎqê iº@H³SÜK@¬M@O¦[¿âC<}‰ÃŽ¿èó|Š¿äw‹pû¯}¿ïÿ݃±Ù_UNASNone@Š:Gy¦µPowerLawnone?ïՓµ?€¬¯Ž_%?u6}àÁyo?€¬¯Ž_%?îkëԂX?·t­Å?©AB¸³Ñƒ?·t­Å?íT"êõy?¢ärÂփú?µ[gG^y¸?¢ärÂփú?íݱöÕo?M"ZË?±pIWü…?M"ZË?ï)n8h?¦aâ(IÐ?šßRC@\í?¦aâ(IÐ?æ²=]Q?ÏmÅø"ž*?Ó›…Eé]?ÏmÅø"ž*?éa)¤?´,‹ð«Ò–?Ê{YŠm‹?´,‹ð«Ò–?ã4åy¨?¶½]q‰Õã?ٗ5¯Ä?¶½]q‰ÕãAGN3FGL J1728.0-6446@tvÌcñA À0MÛU%ÌÀ:¾[
À;¤®ç¸5?™"¤¹É"þ@YKÞzÊ!@Nº€D¿ê$­´Y¿ç8Q¥¿íÀ¢ox€¿ïýb¼¶UNASNone@t{9à`þHPowerLawnone?ïæ['ÿ¤ï?h>*†5?i¤n?h>*†5? ?"AÑ^ì?‡{9ÌCî?"AÑ^ì?îԇ¨o98?'¸,ä×[?¢·…zÄ:"?'¸,ä×[?ï'ÿ?Lr?shÉÓ(G¦?@0& k©?shÉÓ(G¦?ïÏRÀ,ÿ?ß(Åø…?xV h@F?ß(Åø…?ëO+~?čÓüJ?ÃöÃS¯Þ?čÓüJ?íªÎ³VÀ?¤®Ö¯´?²©Q÷V?¤®Ö¯´?çåú±?0J?µ}7÷Ï?Ð4
Ÿl?µ}7÷ÏAGN3FGL J1729.0+6049@Vr¦óõ/Â@@µ‡?úÁÓÀ:WQ§'€¡À;¢µ'ôcë¿ëMT¶T"@ÒU ˜ÑÉ@-ž_§'¿è`
rô5¿á/èSÍÜ¿ìDƒŸÝ+¿áôÉʨŸ
UNASNone@"ßF§ï²PowerLawnone?ïê©4Iç2?¢*o¿¨Í?eVˁ޽ì?¢*o¿¨Í?ïÛe…¯›¨?'ñ™‡¾ab?rM=8°K¾?'ñ™‡¾ab?ïy_'aÂ?"[ïˆkÁ?žÔ
³ÇÃ?"[ïˆkÁ?ïû–à•?3gÒ¢(¦?A¥¿¦v\`?3gÒ¢(¦?ïؗ‰|ž•?z Ï!G™¹?s´;'"­Ê?z Ï!G™¹?ï"«!?­wÁÏåþD?žíj™Td?­wÁÏåþD?í›Ñq'Y?¤ˆð
 zÕ?³!tw층?¤ˆð
 zÕ?ïX‡Ú:¯º?'ÝZUåNt?"︪°?'ÝZUåNtAGN3FGL J1731.9+5428@TŒ]á\¦Ê@@"ð^¢LÇÀ9Ò®Q·'¹À;Ù
£ÇðÅ?ÜÑ-<¬·6@
_hT'I›@7#_ÖS¿çފƒu•¿ë€"È×Ë¿ëÄ@Hq-¿ïþó…?¼ÑUNASNone@tR4Ö¡aåPowerLawnone?ïÝ»bþ8;?sŒ¡¿§þ?q"N"!²p?sŒ¡¿§þ?î'öE¹j?²\ÜqQô?­€›¢±ô?²\ÜqQô?îÍi¤M@"?'|>ƒ¸°?£)e¼ݹ?'|>ƒ¸°?ës{¢¸§?¡­ë{²ª—?ÃÒ2uc?¡­ë{²ª—?ïg
Of?"‰ÅƒZ҄?"^{:§Ô?"‰ÅƒZ҄?á@ƒ"‰Â·?ÒÅÑV°w?Ý~ùºìz'?ÒÅÑV°w?í×zâì–8?¢×ëv̉?±D(ç¿g@?¢×ëv̉?ɎðÖ
à‹?¯Œz¡s?éœCÊ|‡Ý?¯Œz¡sMIXED3FGL J1732.4-2709@v×Ûôˆ@8™aeu¦À8º­²URBÀ:Wè+Íä$¿þëÖj…Yò@"v¸@ûԀ Nj?̧¸ÃL賿ê•`;¿Ýû–EɅ<¿ç"´ìA˜bUNASNone@žõãS&PowerLawnone?ïÂEy?¼—"¸Œ¬?Ÿ‡·dÈÚ?¼—"¸Œ¬?瑩A5CH? ·
Dwƒc?†ToÃÝ:? ·
Dwƒc?ê".éÕú§?±ÛJ²vwe?ųDX¨f?±ÛJ²vwe?ïÿó?Ó)³>áwoqƒŽ>ÙÕRÀé>áwoqƒŽ?ï;w­o?¯#ûøƒŸ?˜Ž!Ѽ?¯#ûøƒŸ?íânTqq\?¾|MeZð?°ì\?¾|MeZð?êŸ{2Õ?°[Ûfü5?ł7Œ«—?°[Ûfü5?ïÿ6TXzs?ócbW‰?5z7Uy¹?ócbW‰AGN3FGL J1732.7+5914@Uøo?Rü&@@ƒô#Rë_À:úkáÐÀ<®âô?¨«CLš@)¿A@S f'?ïŽß{r‰'¿å?Ç7%tó¿ä{þi/¢
¿ÅQwnUNASNone@®;àƒn˜PowerLawnone?ïþ!ܧ=û?4â=üÇ?-â4y?˜-?4â=üÇ?ï×-ÏNº×?ƒ¯á±?ti>…ŒÊ?ƒ¯á±?ﶂ^¥¸ó?|»ú•#'}?'_hNR³S?|»ú•#'}?ïð¡^ÒH?M·}}0õ?^½ÛnVnÿ?M·}}0õ?ïûÛÕ˛l?CŠŽD
C?@©½÷o?CŠŽD
C?îßèÿ™?°^Õ:"}?¢pg?°^Õ:"}?ï^×0¨êE?'"ªëq?Ã?"%욅m?'"ªëq?Ã?ï3šþRþ?•V
äå'M?™Œ .U =?•V
äå'MAGN3FGL J1733.5-2811@vsw[0@#lfZ§ìÀ8Ã=dRÀ:.¾ÐŠÇo¿äРÅœ´@b£S&@é¿¡Á¿ÀŠ»î‹Áó¿ëòƒ
¿åàèϦŠ³¿ã—KOx}UNASNone@ŸIBø7´¢PowerLawnone?èÀaì
ò?ÎJG£'?ÌþxO‹È:?ÎJG£'?ï–ÌW±í£?¤6ºÄeé?ŠLêÓk?¤6ºÄeé?æžt06?·k""X?ÒÃéŸó•?·k""X?ïüú¦ò&?+w/ä2o ?8*ÉÞº?+w/ä2o ?æ1÷Óz½?Î
IQz?ӜY‡?Î
IQz?í_YuxcO?ÁfKêËKª?µ4R…ˆ?ÁfKêËKª?ç´üªÁ?´TýÇyM_?ÑÀ–«Ú~?´TýÇyM_?ïÓì¸c?lb×ÇAê{?v	ñµ(Z+?lb×ÇAê{AGN3FGL J1733.5-3941@uØۋ¬q
Àâ1ƒ/ÊÉÀ9&/ŒEÀ:É+üLû?ÞC+9zÜ%@­OoÔÏ%@×àŽ¾¿âr¶ì€Ø¿ê'WMKt¿Ø'å¾òTؿݨ`'CLUNASNone@£7½Ùb·PowerLawnone?ïùlÞ®)Q?MsÛ  2?JL†JÖÓG?MsÛ  2?ï\hÿ· ?§Ín·‡…	?"²å0v?§Ín·‡…	?P	
?Šëýpèæ?Ùkólix?Šëýpèæ?ïÚä)'Ó?Tˆ@2w…?rô
È.q?Tˆ@2w…?ïá[πþ?pÿi®5°?n¤0Œ¿àc?pÿi®5°?긤|ª(;?Çþ¼SSÿ?Ån
W_?Çþ¼SSÿ?îX—«³? =üM¹‰^?ªvŽ…GÕ? =üM¹‰^?ï#¥Ëù_Ÿ?†:-¹Š ?›‹F}dp?†:-¹Š AGN3FGL J1733.8-6056@t³‰ßrïÀ-‹:%•»¿À9poz^ÙÀ;'2{}NàÀX×æÜBŒ@%€˜Á­_@§©Ÿ¡—¿çN"kô¿æ-ø°R¿ì"ùTs¿¶G€‡UNASNone@'$öݬîáPowerLawnone?ï÷ÕRu?RBÎ/È ?PUï‡&ú?RBÎ/È ?ïÄãW[d2?Žp湏w?}ŽT4Vù?Žp湏w?Hì®?vRrü?‰Ôú\–Èž?vRrü?ïÿÿNK´×>š¤ØÏõ>>–/"ÖOÜÅ>š¤ØÏõ>?ïÌi—:e?~eþB·?yË4uY¤?~eþB·?î€ ¤eO?µùšï±³?§ýõº†íþ?µùšï±³?î¹im6?™ðSX¥Z-?¤n™o5ž?™ðSX¥Z-?ïÿ×åôTë>ÿ¬P`ਵ>ô÷Í7ˆã>ÿ¬P`ਵAGN3FGL J1739.9-3124c@vT&Á½¥¿Ð†êÕÌOÏÀ8\+xSδÀ9ò5ýé?õ€@tº<&@zž¬¨ë@P¿ "_ž¿Ü`7˜r¨¿åӃZho¿çd'²ÕŒ¿èߪ4ùyUNASNone@¢"&€IRPowerLawnone<?¾X®¤»A?Ē‹³'N?ì4ê+hŸ¸?Ē‹³'N?ÞfIéŠ.?ÍÆ"Ž AT?àÌÛ}:é?ÍÆ"Ž AT?Ù¼Ž£hÇ·?µ  œ]½L?ã!¸®Kœ$?µ  œ]½L?åK[ʚÝ*?¬{ürÿ<f?ÕiHjÊE«?¬{ürÿ<f?'éå'xÚ?¡Qݯ}n†?ïh°Ô&eù?¡Qݯ}n†?±;1)NË?ºÄð#X?íؙں©½?ºÄð#X?ÒW$¶åý?µû»W±8?æÔm¤u?µû»W±8?ÉóØxì>Ç?±	jòC'?éƒ	áÄðN?±	jòC'MIXED3FGL J1740.8-1933@º¡<ü	Ñ@NkawêÀ9‡¸·lxÀ:ÚwNëö^¿ý133‰o@5M6¿"»@²¾_v³¿àaKw«:ß¿ç<A³¥£¿áv…¥ñ¿޽çIÙEŠUNASNone@¦
ʦL/ƒPowerLawnone?ïûÏÞhðH?I)#xÍÂ?@À†'Ì!?I)#xÍÂ?ïÛ Ñ?¨,M¢Š?œØ{Û?¨,M¢Š?}:_Å?Š593,œ?W`´×ªÐ?Š593,œ?ïÿúQà>ǽ·#½_>ƹA¤L¹Â>ǽ·#½_?ïô†BWq	?`[K—6t¨?Vózù'ï?`[K—6t¨?íW8ßM5›?¢ìVR?µF9à-£?¢ìVR?îŠ@,.Ëß?ŸZå¼£X?§[ý>Ë?ŸZå¼£X?ïÿš¬‹†(?
fLÔDm?	TÜí3ïÿ?
fLÔDmAGN3FGL J1740.8-6755@tRg ù	lÀ2¼8…	ÀÀ:Fšï/À;»\´5ýÀy
‰ò@`›csAì@O蠒Ý¿ça¶u¿èÇÖñhãn¿á'Ú~U	¿æ)wT—©LUNASNone@†Œ0݂ývPowerLawnone?ïîîm¹õb?¦ËuÈ6D?a'~d5g?¦ËuÈ6D?ïÇ%ÉÆ»™?Žlé+?|m8Îÿ0?Žlé+?ïсèՎ?|¶x"™à?w?mX¨û?|¶x"™à?ïÿûÌVU>¿O6ÇeŸÂ>ÀÐtY™ùi>¿O6ÇeŸÂ?ïþä‹ýœ?$†um=/?!·=-a±®?$†um=/?îš/ÅÚ.#?µ"dó'?¦] ¥OÑ?µ"dó'?ï¥F-d?†§v¬"Àò?†®t»÷d?†§v¬"Àò?ïÿ‡êÆ2?Ýíœ-Kt?>úlº€??Ýíœ-KtAGN3FGL J1741.4+0938@@âñ©ûçm@3ãý?[_¢À9vèõø?AÀ;1ÿD]Å?íº^?rÓÿ@À9Iøœ‰@ø8`nª®¿ß؎Éöj¿ë¤g¥£	§¿èpp3 …¿ïñ'½pI¥UNASNone@~
d×ðíPowerLawnone?íõõBÑ{?¬_hãq¾"?°W U
,?¬_hãq¾"?æÅSÚ{>Ã?Èj¢`<«­?ÒuXK	'z?Èj¢`<«­?íVöو'?¡x"àNF?µHI4-Wr?¡x"àNF?èBÁMµ?¥ò.R›$Ö?ÎöúÉ+Ð?¥ò.R›$Ö?é…Z—ršI?Â/Ì/‡ÆÍ?Éꕢ5–Ý?Â/Ì/‡ÆÍ?Ð-!¨¾?Ìó.|Pn¿?çéo+ ±€?Ìó.|Pn¿?çÌ?»¤'ß?¶&ry|ë?Ðg€ˆ·°A?¶&ry|ë?ÍB¡BãÞ?­ ©G%rD?è¼oW¯G	?­ ©G%rDMIXED3FGL J1742.4-7237@tgßã*À4à´Ê!!À9ùÖÌ*žÀ;¸ßR,¿ÞÞxžÕÌ@ 3&H@aÌà,¿ìé܉ûŽN¿èú¬Èº2¿â2úûM,¿å»¢ÆBUNASNone@qvLáłVPowerLawnone?ïþŸº'Z?8vaoúŽ?&Wò;?8vaoúŽ?ïÁsËÝA?rß#D0d?ƃ{y?rß#D0d?ï¿#=>F?ƒ¬‹!ÓX?€?w'†w?ƒ¬‹!ÓX?ïöŒ¬Ô½e?>þG…©/?R榶ºF?>þG…©/?ïü×Ã5µ?Be+"X?9Aæ
¸Šü?Be+"X?î7O$øª?¸.±	ËüZ?¬ŽûûøV?¸.±	ËüZ?ï£CÐJ–ã?ƒ@j›*Ƅ?‡/æ{9?ƒ@j›*Ƅ?ïwNÞ¬Á?'7¿M@?'–"aû?'7¿M@AGN3FGL J1743.9-1310@*«ø˜,²@ õµØ",À9†·5ŒÀ;
3­¬v?ñ5£Ãi Ö@ó»Æû}@ærÀ'Ö¿çpïñü¿¬ÍÆU;%¿äv–9½»ã¿í¬ŸâKgUNASNone@Œ‡"ݘPowerLawnone?ÄO4Óh¿©?Ã|9°ê‡â?êì2Ë%Ð?Ã|9°ê‡â?ä~à"ðò?ÎÐsU7??×>÷À?ÎÐsU7??ãÎFî*?³qK2SE?ØcsÈ#Å­?³qK2SE?è ç>›¤¿?§ùŽb3ì?Ï|c'm?§ùŽb3ì?®36¨?¶J#?VIf?îõÑu?¶J#?VIf?Ð7:Ï^Ík?ÎÛpžÎŒÀ?çäb˜P™K?ÎÛpžÎŒÀ?Ë£*­ä»g?¶'É6Þ?é5T†Ñ&?¶'É6Þ?Óu6''#I?²ÒӖÓ\,?æEd¶ìn[?²ÒӖÓ\,MIXED3FGL J1744.5-2506@	0"¿íÁ9@¤±«VçÀ8&ÆÌ˲À:)}uv¤¢?Údúr™Çß@
Ó:ÉT;@‡À(N©¿æšø2šö«¿êñísˆ¿ã÷[ Üü<¿îart`UNASNone@ˆŠ$tSŽóPowerLawnone?Îþ¹µ°H?ÎéÖü¦"?è@Q¹R"î?ÎéÖü¦"?íºí^#?Àe"•ý
‹?²/X•êÎÆ?Àe"•ý
‹?áHIúc͟?´û.!5
Í?Ýol8dÃ?´û.!5
Í?íÏ©¡¾E?•ýÄ à3'?±‡ÚµÏU?•ýÄ à3'?Ñxòp±%?ÌDeø#ßû?çC†Ç§@n?ÌDeø#ßû?ä>~P±ã?ÒXÜ¡Î?׃^œ:?ÒXÜ¡Î?ã‰wüc?µ×š4ûÞ~?ØíÎÅ9?µ×š4ûÞ~?âwæZ×+?·q÷%>h?ÛÖ3JQª?·q÷%>hMIXED3FGL J1744.7-3043@vfÃóà7¿ès ôlNÀ7þ+i:V=À9Æú¤vln?î&U)s@F¬RÐÝ@æ›_Â]]¿Þúê—c	¿éðŠtÁ%­¿äÞ—fñ¿èÕ¨5
EKUNASNone@žº±ø .PowerLawnone?Ì+aö´9?ÌÔ{¥ž?èõ''X'ò?ÌÔ{¥ž?î'\[±½¹?·#Ùß;µ?­Š:D=r?·#Ùß;µ?ÚѬj¬œ+?¶-½R†`?â—)Ê©±ë?¶-½R†`?í®Jq?¼'­U»?²‹÷o¸ü?¼'­U»?;#"Ë_?Ë=k€4?èwÍ(?Ë=k€4?߶¶I†?Îlk–¯Œÿ?à$ñ¸$Û=?Îlk–¯Œÿ?ٝ£"o8?¾4ˆÎVv?ã|±.5Èd?¾4ˆÎVv?䋣ÛŸA?³×5gˆ(?Öè¸IÌÁ~?³×5gˆ(MIXED3FGL J1744.8-1557@&™»'ˆÛ@€ô"'òÜÀ9Rìzçý«À:î__áçç?å+Y Çd@ö–²‰›@z‡`%¿©ê7'õƒ¿äõþš'Ö<¿åjc㡜ë¿î–"	u°ÂUNASNone@Áñ©ûçmPowerLawnone?ã¾ÙñÒs?ÓXÈÃþœþ?؂Lî[?ÓXÈÃþœþ?çtý› Ø=?Ë°àóuX?ÑɾO†?Ë°àóuX?æ×{äÿ&?±ÚÊ3¼ÜD?ÒQ	ò6³?±ÚÊ3¼ÜD?éM
•Îé?¤rWµnmc?ÊËÕ©ÈÄ]?¤rWµnmc?ԗVh—n?Ï¥(v–µ?å´TË´Hò?Ï¥(v–µ?ÓÉÉsb4?ѲøÙ°W?æ{›FNæ?ѲøÙ°W?â#ä9Œ#ö?¹"Ԃ·?Û¸7Œç¸?¹"Ԃ·?Ð~÷Šn6?¯ÝíŽa£?çÀ":Èäò?¯ÝíŽa£MIXED3FGL J1745.4+4721@R'±F^‰"@>n9`sÞÀ:'ó²ê£À;Í
ÌÜ­À÷l–\ò@ªõ «†¬@wàyQû¿å`üŒ&¿éª¾UÌÌ]¿èHˆ&w'¿¨'‹‹ïøUNASNone@ƒô¶E¡ÊÁPowerLawnone?ïÿœZ" 3?
2'ö̂1?éd0ÒS?
2'ö̂1?ï݋ÈùÐ?'•«Ü5?q:øãà?'•«Ü5?ïÖ҂?uŸö·K@#?tôü¬¼s¨?uŸö·K@#?ïÿÿÿv¡>$yÕ\;»>¥Á£¥]Ã>$yÕ\;»?ïÿwnmé4?05Å®&Ú?4Wsú,?05Å®&Ú?ï(ùMUÀž?©€@jôؔ?šàÖZoV2?©€@jôؔ?ï'Õçõêu?ˆ·"94'?‹J†…bÍ?ˆ·"94'?ïÿÿËìkè>ž$ˆ\Áª>yèWÛs˜>ž$ˆ\ÁªAGN3FGL J1746.6+0433@="¿¤Æ†@0}­ÙÂ~•À9œ-~¾LÀ;*þ±KÀúð¦ñ›ä@
{«lù¨@Ys_ÉZ¿åÇ\R׿ê¨Üäá°M¿ÚÖ\j[Šã¿é–è4l×UNASNone@Œ×oiPowerLawnone?ïîI?ÉÏ?ƒo?æÂ?a¶Á"‰A?ƒo?æÂ?ï¨äq{s?•©K¿üAË?…Æã´ë6?•©K¿üAË?ïaKdWmz?	Àmú̓?"Ö"n3Ä?	Àmú̓?ïÿ÷BÛá>×Là!ž5,>Ñz: õï™>×Là!ž5,?ïÝMç6ö?{è±.Ç?qYv³ù?{è±.Ç?î™ù]Eù?»E%A5²ó?®F`hsÒx?»E%A5²ó?îyI"®o?›<•P—n²?¨kfŒ?›<•P—n²?ïÿ'ôsÈ? -ìÄÏJ?åýÍä? -ìÄÏJAGN3FGL J1747.0-3506@v.cÇOµÀ§|{{¡aÀ8MRÓâjÄÀ:²	Bžá?ãšÛ—&3@ª½ÐZ¡@UÝw"q¿æ}"®î¿éÀ¬cÜÚr¿æa¶DU¿êaé©sΦUNASNone@NÄÑ¢PowerLawnone?íÄb$ã9K?¿Š±/ž^?±Üî×.g¬?¿Š±/ž^?îϝ`åh?°ö¨
Èg?£*^|?°ö¨
Èg?ìƒjÞñ?«Ad¸âQ?»çü©ws?«Ad¸âQ?îˆg© +?†}¤ê‡R,?§yˆÕ™S?†}¤ê‡R,?íkÊ´³j?·_=ñ/á"?´£ñ¬2¬?·_=ñ/á"?ã>ŵM̉?͉?¢_ï\?قt•dfî?͉?¢_ï\?åï=¨,.‡?¹Yu6¬È?Ô!"¯§¢ò?¹Yu6¬È?å>Zcžœ?²S½ëì?ՃK8ÂÈ?²S½ëìAGN3FGL J1747.3+0324@<›0aǛ5@/—Õ#³coÀ9iRÍ,nÀ;âµl]÷?¿€3¨4MK@
ã¤)Àn@Õ€ÙY¿æj2X¿âZÍÖâû¿áb¾Mz~™¿îWÂ?'K©UNASNone@˜5å`A‰PowerLawnone?éÉ`ðkô?ÂÌrŽ+Á?ÈÚ|>P-ü?ÂÌrŽ+Á?ïJ]8ë.?©ž©ûpâ?–´Xàâpˆ?©ž©ûpâ?ê[Ž˜Mƒ?­§ÉÆÓ¦•?ƑŞÉóî?­§ÉÆÓ¦•?ïTRÛLË?{GJùï¶Ú?•}5¨ž?{GJùï¶Ú?ÝRʕîqì?Íc¥ä" ^?áVšµÇ
?Íc¥ä" ^?ë&äRFì?Æt_,?Ãdn¶äO˜?Æt_,?ãþRÛ¸?¿%´k=K÷?ØZIïڐ?¿%´k=K÷?éÄJÔ«ò?³C¶ýÇZa?Èî׬­P8?³C¶ýÇZaMIXED3FGL J1747.7-2904?À&'j(¿ÞZº LѕÀ72_½‹çÀ8í¸_~?ò«Ð}ÜO@·ýÊñ€`@ ?Ðû[¿â'†Là®V¿åÐ܎¶¼•¿æƒú¢Ý÷¿ê¬;ۀøAUNASNone@¡2a|ÚPowerLawnoneP?À¶…Ìþæ?Æö/ZOq?ëÒ^¹ÀG?Æö/ZOq?ëé³y·Q?Åð'<8s?ÀY3î"¼?Åð'<8s?Ôz_]™ÊR?´=¸1:ê?åÂÐQ3×?´=¸1:ê?ì'LY±†? š@ûÇ?»u2wÃÓ? š@ûÇ?Ì¥hý­?Ϛe!þé'?èÖ¥À»¾Õ?Ϛe!þé'?áÄY»"Ø?Ó	ɦìWE?ÜwL‰ÖP?Ó	ɦìWE?ÔéhLñ?¸$à¨)‡ì?å‹1KýYˆ?¸$à¨)‡ì?䰜s¤Î'?µê¯'̝\?֞ǶbÜ?µê¯'̝\MIXED3FGL J1748.0+2701@IêÊÿm3	@9\gßã*À:H—hfñ§À;ˀ
|ZÄ¿ô=$*ך@
֛	Ü!Ô@8Š`¿Z¿åùzíSwn¿àC8P Îº¿é¹">o¿Á¾ºì¶³AUNASNone@–/&€IPowerLawnone?ïø®DÿH?W<©9+é?MFïݾ!?W<©9+é?ïżƫ†½?Rþ±t¢V?}!œ²{±]?Rþ±t¢V?ï/ú]mˆ?"ÒŽ¨…âÜ?´^UÊ?"ÒŽ¨…âÜ?ïÿÛ§}T>êÏ;ŽÓ.·>ò,Uþøf>êÏ;ŽÓ.·?ï™'A@Ô?A¿´}ê?‰¶/¢;
?A¿´}ê?î-µDðË?¸u¤¯¾?§
$¨AWW?¸u¤¯¾?í"T¤`â?«y¥udã?³ß=Zos?«y¥udã?ïû\ʱ>§?EpU
Ǭ?BŒÔÙ*º?EpU
ǬAGN3FGL J1748.5-3912@u÷ù=ÙcÀAhr° ÅÀ8סÙÙû‰À:ø
ºÓ¦?ðofÈ61@œ4¡rV	@mŸ€8t'¿évq¡Wþð¿Ñèß	Ü5¿ç­o÷¿ì¨Ð%Ǻ¿UNASNone@"‹)^žPowerLawnone?Ñi¬/ãl?ʬŽ•üÎj?çK)èzJ?ʬŽ•üÎj?äNüˆ¸\?ÈËù=!?×bîGå?ÈËù=!?âŸ2&\¤à?´ÆøÕÐa?ÚÁ›³F¶??´ÆøÕÐa?æg^Š
@²?¦H…ErÓ?Ó1Bëë~œ?¦H…ErÓ?§Q¸TP×a?²ËÈeÀìG?îŠäzñìJ?²ËÈeÀìG?º%U9˜R?¾b{Œ ?ì»UXÌõ½?¾b{Œ ?Ì£ÓË)ð¦?·‰D¿éÃ?è×
5ƒ×?·‰D¿éÃ?Łš¡xØ{?¦›Æå?$ý?ꟙW¡Éá?¦›Æå?$ýMIXED3FGL J1749.7-0305@6ú¾Yl'à@(o:¼"peÀ9,AˆaÀ; ¡`7x?Æëñ•®þ[@ß9Xç!ã@fÀ_ñ¿ë Þ®ÁÊ¿Õ@ÆÚ'w¿ç‡½;èÁþ¿íË !³ƒûUNASNone@Ž.49XbPowerLawnone?ހ	‹û?Ϊ2@øvQ?à¿û}º@?Ϊ2@øvQ?ï¥f+ƒ?±Y1¼ðÊ?KS=ÿ9è?±Y1¼ðÊ?æHaÚӇ?³1˜?Óo=ÎJXò?³1˜?ï#ÿº"‰?€ûºŒ]?›€¶ÎVç?€ûºŒ]?ÏÛ)u³û	?Ë|ÆY–}?è	5¢">?Ë|ÆY–}?ê/{e¦øÓ?É^ŸâLՊ?ÇBidµ?É^ŸâLՊ?ßµaf!r?¾ôå*ø¸I?à%OLïFõ?¾ôå*ø¸I?çX:|õì?µP¡Ýþ
?ÑOá‹'?µP¡Ýþ
MIXED3FGL J1750.9-2220@ö>¶5@ðï ´«nÀ9³Ët9À:oóþj¿ýQÃI@eÌ@AþíÜ<@¤hŸÑ—¿æ6ÈG'¿íáÇï~Ž·¿¯¼ äôXN¿åO¥&À‰UNASNone@˜==Ùb·PowerLawnone?ï~lHä²?œ¼bpÆé?<Òp1Ù?œ¼bpÆé?ïvãú:ï?¦°g½-¼_?'#€¶êOy?¦°g½-¼_?ì»Rn`)?©c»@|T·?º%läþ·?©c»@|T·?ïÿ÷Ò4Û>á~<ªbµ>Ð[•/ð-˜>á~<ªbµ?îݍSdù?«P…÷?¢'.L~i?«P…÷?í/K¡WíÁ?Ãœ&wÔ?¶…¢óö·v?Ãœ&wÔ?ì9	¸%Ì?«7Ît(7?¾7·Ò>Ñ¢?«7Ît(7?ïÿ»™kó?}{'sþ? )Ø£?}{'sþAGN3FGL J1754.0-3321@vQú¬Ùè>À'å=ÌÀ8çj"ò¬À:·D[y£Z?ò¹ÊE
@­\7äH@K?ëÓM¿Ëý4±ëþt¿êGVù'¿àÜÔ2Wý(¿ìý‹UNASNone@' ù	kºPowerLawnone?í–Ö͛mž?ºë»'«?³II"Üa?ºë»'«?ëR‰Cyì?À)4ÞY?µÚòOœ?À)4ÞY?è71BuÎí?±63rè?Ï#:ö(ÄM?±63rè?봟Â'­C?›÷BÖº†?Á-€÷aJô?›÷BÖº†?å"AP?͕:ø'î?Ô×}ÕÃÁ`?͕:ø'î?҈ÉW¢SR?Èm¿‹›ª?滛T.ÖW?Èm¿‹›ª?Ý¥9‹­?¿G˵dj'?á-tc:s*?¿G˵dj'?át.Û,-}?·Ð)<õò?Ý¢I§¥?·Ð)<õòMIXED3FGL J1757.8-3126@vsC•Àv€®ç	À8ÞæïÁõÀ:¢MùÇ?ïÝæ"bè@
6ÐfŠM¡@[,å¾`?ýGªí¶ž¿é^¡i5Š¿ã¹ÛGR¿¿ìÔ°Å@w¦UNASNone@":¸ºÇPowerLawnone?Í2bfx?ÊÖ\ñ*$?è³g&aû?ÊÖ\ñ*$?àßü¡.ä?ʊ¸³ÃÄï?Þ@ò½¢7?ʊ¸³ÃÄï?á¹Ð[L¬×?¶ûÈ0šwq?܌_If¦R?¶ûÈ0šwq?æ'˜5ýy#?¨Ü;ô¡?Ӱϔ
º?¨Ü;ô¡?¾&lÌìW?Àœ»?º3?ì;2mæbu?Àœ»?º3?³›Çî$ý?¹"€5x?팇y5 ?¹"€5x?הÐ4hðã?¹…>_¢'?ä5—åˇ?¹…>_¢'?É"¯o*?ªÕ©Íà?é·y$5{?ªÕ©ÍàMIXED3FGL J1758.8-2402@á•a%´Å¿¦7½D†À8c˜¢ù"¬À9æ×5??ðíäI–!@Yi}È?ÿæÀ'¢Ü?辶ÈèLì¿ç&k
·p¿ÑgîõX8¿æžºM8UNASNone@½ªsa@OPowerLawnone?Ü=‡TȄ>?зF5Ìô?áá<U›½á?зF5Ìô?í»®[6v?ÄËIùâôE?·'""?Í?ÄËIùâôE?ã·qµ
I–?´õs¨OÑ?ؑ•ëlÔ?´õs¨OÑ?9
¬€?Ž¶·"?¦µlkµœ	?Ž¶·"?ÜWo
æå?ϑ'¸›VL?áÔHyþŽ?ϑ'¸›VL?ç<79áð?Ь‹¹²â?ч'ö<!?Ь‹¹²â?æ:¬+l•U?µ9t®½=?ӊ§©&ÕW?µ9t®½=?í	¡ì"+?¤ô¥…7?··RñwM«?¤ô¥…7MIXED3FGL J1758.8-2346@ÈëÌlU?´Ê¿_»ýÀ8^@'7|À9Ǩ§b°?ó›÷Aë]@
Üçl`Px@£¬ "Úƿ©ço?ï•ç·B¿äï]+»Uè¿ä&VÅ£RUNASNone@µ/1A [ÀPowerLawnone?ÁÑ7³©ï?̦Ýáu?닲º?̦Ýáu?ÙI}Ê'£T?Ò¬<	¬¸A?ã[Aì.V?Ò¬<	¬¸A?Ûˆöªä?¶~}ÿø,Ô?â»ù"ªŽ?¶~}ÿø,Ô?äY-è4v?¶Cà4]ª«?×M¤/—Ð?¶Cà4]ª«?Á:âôo?Å-ú"k	8?ë±G}Âùd?Å-ú"k	8?Æ|Xb
Ç?Íc
š·Ã?ê`éç\<Ž?Íc
š·Ã?à?R%g?¹óC'?ßÝׁ[µ2?¹óC'?ÐDñsl«œ?»€ž©vÁ?ç݇FIª2?»€ž©vÁMIXED3FGL J1758.8-4108@uì²êòÀ ÷W÷7ÚbÀ9Ÿ"!°SðÀ;OrSÍÝ?ð9ýŒÞ[@¨¢?¢§@ÓÙ m2Þ¿ÝÔR}%o¦¿›÷Dg"¿å÷
€û¿åm|^ªöUNASNone@¢IúáG®PowerLawnone?ïåq³ÃÞ´?t)r|`¯?jŽLK?"ô?t)r|`¯?íLQîô}?¶*'å?µpº6˜?¶*'å?îè:|õì?"rAxá·A?¡X0¡;?"rAxá·A?ì‹
vÀ??"c»';&?»§¬Iþ"?"c»';&?îJÂL|k?²'&¥ß?«SÛ;¨â2?²'&¥ß?×4Cț~?˪QBóH?äeÞ²@¸?˪QBóH?ëo培?­þµÜ~H?ÂC¨k™?­þµÜ~H?ß|ª…¥?´E>pbš}?àAª½-r?´E>pbš}MIXED3FGL J1759.2-3848@v0@9«óÀ´ãy·|À9qiiP%²À;ö¬š'^?ôÑïK|Ö@×ëϜ`@ãéÿ"S?êužåÞÁ—¿ÞWí',Q†¿àRcz¬L,¿ïÿû)pU—UNASNone@E§8}¿PowerLawnone?Ô½Køå?ÕnUj	
?å¡Zñ@
?ÕnUj	
?¶ÈZ*c˜æ?ñjŠ|4?í&ôºÁKS?ñjŠ|4?ۃ_kˆ±?´
bšlô?â>PJp;§?´
bšlô?ÒjFCR²?°0­É†¯"?æÊÿÜÞV§?°0­É†¯"?ÍЧ¶ŒQ?Ñ+G²Ø@/?è‹Öy\ì?Ñ+G²Ø@/?—äL<»êt?±5‹š	"?ï@ݝÕh}?±5‹š	"?¾ò³;VB?­g–€;?ì?A©˜•8?­g–€;?«&8¼ÉšI?—60~þ?îMœt%§ë?—60~þPSR3FGL J1759.6-2141@dÁr%·?î¾UíQÀ8ªO¨´¿À:0``'çÏ?î4)¼«±8@ò҈"£Ä@Ks«¿ìMÃñö—¿â¦â+]¿â¬Ö²°¿èö® þìôUNASNone@¥ƀIRPowerLawnone?Ôx5bÚ¸?Ò^Xì¼g‹?åÃåN'£ö?Ò^Xì¼g‹?ç¤mÿH0W?͌#q|Î?з$oŸS?͌#q|Î?ã"$jÌY?¸$+íê_Í?ØÙ·*g÷O?¸$+íê_Í?ê´¢PRw?£Á~GÖÖ?Å-v¿¾¶#?£Á~GÖÖ?µZIÕ9—v?ÁʀAXæ?íT¶Å=P1?ÁʀAXæ?Ñ)ÏæÌl?ÐŘvÀ?çk™Éô?ÐŘvÀ?ÞAÄ­»ÜÝ?¹%ð	ÕÑ4?àß©"'?¹%ð	ÕÑ4?Ùª—mÕ_?¶½Ò½ñu?ã*´wIP?¶½Ò½ñuMIXED3FGL J1800.0-2955?çò–öQ*•À	¼©ïR2ÓÀ8®ñ7æ [À:k¹8›R?ò¦©½S2,@Å2™Û2ì@N5gÙÙ¿Ô­æ¡Îá¿ê²ÞŽ~ˆ¿ë'ÏÐã1é¿ãʎÎ([XUNASNone@ˆwÄg8~PowerLawnone?éo‡Ù—zI?ÉSO¹·ØZ?ÊAà™¢Ú?ÉSO¹·ØZ?é·™£™g?ÎEßí)ÓR?˵!™qšf?ÎEßí)ÓR?ç¦gq9T?³Û¹œ?г1ŒáX?³Û¹œ?ë߈.ôEs?¢'ÝܖMÈ?ÀßD.ê4?¢'ÝܖMÈ?ßïK¤ï?҅¼âé·?àuZ}­ˆ?҅¼âé·?Շ>?M?E?Ò ×î`gÁ?å<`àY`]?Ò ×î`gÁ?áè#û\Ø?»dÆöky?Ü/¸	FOÆ?»dÆöky?Þ;ÛÊ®Å?Á0X¤ÿÓ?àâ:¨?Á0X¤ÿÓMIXED3FGL J1801.5-7825@sµ4'¾‹ÁÀ8b{öÀ9t¢ŸÒ™À;?Mó¨Ú¿ë)Ԓhø½@ó*ÁŸ@	òŸÅ,Å¿ê[i1¿7/¿ç@.·V §¿æ
Ðl-j¿ãOïáêtUNASNone@yÕÎ;Í5¨PowerLawnone?ïÿ²y~4þ?@(¸ý@?a«êãGÆ?@(¸ý@?ïʤ󃴚?ŒËÛ
d?z­†@5w?ŒËÛ
d?ïÝ¡rù><?ghÓ೦?q/FcÄz?ghÓ೦?ïÿ˜ÂaÂp>ú`«>
v=?	Ï`Ü&ò‰>ú`«>
v=?ïÿ…£1a¼?+ƒÞg(?—#Ï°2÷?+ƒÞg(?î¹X4Z¶Á?´‹p',?¤j|¹x¬ñ?´‹p',?ïćfï«Ó?}zйÒP?}¼L¥Γ?}zйÒP?ïúßäM?<G01	Ìo?Dƒ³gv'¨?<G01	ÌoAGN3FGL J1801.6-2213@uw¾}~±?Ó|½U`"¥À8ÔQ ˆ6À:1sˆÙ?ㄾ2Ö"@
†ÆÎ[S?ÿ{vÁ'}?ïò"c"'¿Õ89Wd•×¿é'L"5à¿ÃÀdÿðUNASNone@À‹ì(õPowerLawnone?ä'ä›9?ÑNë³W ?×Á±þ6ɍ?ÑNë³W ?Ži˜S?½"¯m?¦"GfzÖ?½"¯m?å—ìGˆÍ?¶Æ¨=Œ?ÔÐ'pîeà?¶Æ¨=Œ?ï³|Ú¤¯U?sËR—†'Ð?ƒ ÉK}tÒ?sËR—†'Ð?ÍZS\?ˆÔi'X?è©xk:zi?ˆÔi'X?ê0ºÜE¡Ü?Ëï£uLÖ?Ç=Žéx?Ëï£uLÖ?äü"°Ñ™?¶ŠU[‹×?Ö֞\Ìà?¶ŠU[‹×?í°ÑxFýY?­$!±üH?²yt<G8?­$!±üHMIXED3FGL J1802.4-3043?Óqº™MÀ7%_5½À9?»vc3¬À:ÞùN59?èÒD–ï@
}XsI@â°À|²X¿éþ*7Œa¿à"…‹ð¿Ñ2©gR»¿çy‡‹ÉDUNASNone@ª£n.²PowerLawnone?ïº$'Q¦?¢
¹—ê,?vß\ÕĜ?¢
¹—ê,?섂­]µ'?śoõu&?»Ûê•Só?śoõu&?î,·FäÒ
?¢ñ@k?­4‹*-?¢ñ@k?íõ™²÷?'aVøÛL?°W7"tÆ?'aVøÛL?îΏ¼îTÔ?©ëڄOÃ?£-«Á?©ëڄOÃ?áLÖLIÑþ?ÒÆM|_¡ü?ÝfSgl\?ÒÆM|_¡ü?ìj,⾄?ªv‡­?¼®Ÿ`êÞ?ªv‡­?ç™@€9	?¸ÀµdSÑ3?ÐÍ~ÿˍï?¸ÀµdSÑ3AGN3FGL J1803.1-2728@	ÄÙÆ°SÀ³#»ÆëÀ8õ	¾ºÀ:ŸŠÙv0?æàK£R¼!@0î™Ñ!ñ@°yݽ¿èBšëdx·¿ãðd@"»V¿ç
zÎ
¦¿äâlÊ갟UNASNone@œ+C,¥PowerLawnone?ïû&ô­ß?«(ê@6b#?À›BÚ/?«(ê@6b#?îBŸÝoK?À|?ÿÒç!?«ÞFM$N?À|?ÿÒç!?í/ÐÏT«B?¦ÐÝPô&g?¶y…Z¥ñ?¦ÐÝPô&g?ïL"ñ§?xóŇM¯"?–~¢á?xóŇM¯"?æÊN/â+?̵¬'š?Òkc ä;©?̵¬'š?çÛ·ñÉ[~?Ïӝ
8ð?ÐHmI?Ïӝ
8ð?æ\ÌQìv?¹Š%33^?ÓGúg\'?¹Š%33^?ë3édï))?«ÊID)–?Ã0ZlC[[?«ÊID)–AGN3FGL J1803.3-6706@tmã}é9ëÀ4^,ýxÀ9†‡OêùÞÀ;§âïÙ?âÀƒ!w@ΰýŽa@»_ÛÝ·¿ãâ݉¢D}¿á-0K'Ï¿ã®1]›¿éí.ÔßôUNASNone@•iᰉ PowerLawnone?ï‰'ôE¼?§ôë}ü%?¶\œí?§ôë}ü%?îØõЄÅÖ?¤@O/õ¹?¢p¢ùkp¤?¤@O/õ¹?ï>Èʁ?'3õy4…?˜&檶¥Ù?'3õy4…?í1óé­ik?'(R­Âˆ‹?¶p`²"´¥?'(R­Âˆ‹?ëï¼¢d?º"=^Q¼X?ÀA
wžp?º"=^Q¼X?áèIï§?ЙÝ|†?ÜÄ/l ±ô?ЙÝ|†?êÙ"~­0?²Â´£"Ì?ěvÉKA?²Â´£"Ì?Ü‹&dBË?³±–TE?áòºlÍޛ?³±–TEMIXED3FGL J1804.1+2532@IÕcíb@5*ò¥¤i×À9Ä*lEÀ;˜€LÁy²?ï¼ú@ÝÂ2…@µŸe`'¿äë]ÃÌëM¿î›"rëÚÚ¿Â5¤"ÿY¿ïÿÓÉ&‹@UNASNone@|P…œŒ"!PowerLawnone?ïê?ô╌? .žc'Ü>?eÀìT)? .žc'Ü>?ì%<ç£#?¿–>VŽ?¾ÓöÂæç?¿–>VŽ?›ï	?•§êLÔ3?¤¾ö÷öi?•§êLÔ3?ìV;U8
/?£ŸñÇ^÷þ?½N%V?–ˆ?£ŸñÇ^÷þ?ïãÿŸKÏ?sX&3"È©?læ8ع=?sX&3"È©?âZ*Ìdû‹?Ñ:Uç=;?ÛKªg6ê?Ñ:Uç=;?ìížaª?®¼BfÌ?¿H—3ò­?®¼BfÌ?åfŒdZ{)?ÅdEŸ=ë?Õ2ç7K	­?ÅdEŸ=ëAGN3FGL J1804.5-0850@3¦Rz WŽ@ôº"»äGÀ8¤3¢Ä»†À:¿b֎í?ÛÆ:{?Ö@§!lŒE@þÏ@šyé¿ìâAa&ê¿âÅÝCVZÄ¿á"
ëiß±¿èÍ/UNASNone@{*¹à`þHPowerLawnone?ïñ}7ۅð?\½<Nwä?]®¨S?\½<Nwä?î»°hEÂ5?¸#>n[Å|?¤DùzÇõ·?¸#>n[Å|?ïÎd°?•&¶ì•F?Ÿ_æ.B"—?•&¶ì•F?ïf»eé‹?u*{û¸@x?"=¨Œc–¡?u*{û¸@x?ï,rR
—f?œôõÍÜs?šqµ¹…©??œôõÍÜs?é¾x.B'(?ËcN»Ç8[?ÉFõ»a?ËcN»Ç8[?ë¦Befra?­7³V¡OÛ?Áföjf6|?­7³V¡OÛ?ì$¼ÎZŸ?¦×Ž†eì5?¾Ú+|?¦×Ž†eì5AGN3FGL J1805.9+3407@NGæÿ}ú@7¦êÙ'N#À:µ7"Ñ‹À;£Ò$ûb?ҜkÒGFL@3úkU9@Êî «†¿ãå~'*ð¿á©›yÙ¿ë‹<7yúÿ¿ïüO¹ÑlUNASNone@††]>Õ'åPowerLawnone?ïÇ[ÍõÛ~?'"5–$C%?|R=?'"5–$C%?;DÐ?™QQþ»·p?‡ùB\Ø?™QQþ»·p?î›Û%³¡`?"^Þ÷?¦BM¢25?"^Þ÷?ïUñæâ£?vˆH$9ë?•_Ã#«¬?vˆH$9ë?ï5'k³z? åõ~üó!?™M¼«ªXÓ? åõ~üó!?íL¿²n?¿0ß=_(|?·7uœ(.?¿0ß=_(|?졓|ZTÆ?§;@»å|z?ºód-YÍ?§;@»å|z?èˆÚ@öØ?²ÿ$÷>[?Íܖü'С?²ÿ$÷>[AGN3FGL J1806.2+2744@K"BJ'k@5ƒ
®>lÀ:w`‰­"À;¢bAQ?ìßôi@X@!eIZçØ@ÆlZ(@?ÀkQF;¿í@Y?¿Õ¿†nª¾Á¿íÞES­b`UNASNone@Š!œ]cˆfPowerLawnone?ï#v6èõL?¡I«?•^?›'9+x\f?¡I«?•^?ìØ?pŸ€?¹"饞Ö2?¹>€¬Þ|?¹"饞Ö2?ì¦Dé'Õ?¦
´¸#µv?ºÏ-سéZ?¦
´¸#µv?ì4L'µ? ".ì2a?¾]›o:S? ".ì2a?ïQòJ#©l?¡?·–}Ý?•Á¶½B v?¡?·–}Ý?âÍôk20?Ï~Κµ×?Úd)šá¡?Ï~Κµ×?éΚ1Äô?³v¸Nû9?Èŗ8ì/¿?³v¸Nû9?âÝ|¨>O?À:*õ)Á?ÚE¯Çƒb?À:*õ)ÁAGN3FGL J1806.7-2451@"K3ÚùÀî['ÍÍÀ9;ofÀ(zÀ:ywÞ]îÉ?èÞÎÆ2e@
×Tª1@«å÷1¿é–´~¿áP²êšàc¿ìÖ;Ÿpý¿¼ß¢-«¤UNASNone@¯='ÞÑ·PowerLawnone?íØA«N«g?¹Rg½ê¶â?±=ò¦ÔD?¹Rg½ê¶â?î]Ú²y˄?À6wÅM@i?ª"TÙ?.¼?À6wÅM@i?éÝuŸ?°•'Ø>Îz?Ȋ+§ùƒº?°•'Ø>Îz?ï«,_j¯Ý?w+ 
\¸?…4è4µ?w+ 
\¸?ßîãRuBÍ?ÏITœÎ"?àŽVÅ^™?ÏITœÎ"?ç½­ð"¦f?ЕÛðB7?Є¤س5?ЕÛðB7?åSP)c%¿?¶Ù3y´^Ý?ÕY_­9´'?¶Ù3y´^Ý?ìB¸Ÿ^œ?·8¿}óž?½ê;=#?·8¿}óžMIXED3FGL J1806.8+5346@Ty
®>lL@;ÿ:Þ"_¦À:#éõÒ"À;ÛzMÝÙÀˆ6Pôå@Ô(ú@@… =w°¿å«lˆûwì¿çÛ×ϊAb¿êy£¢†þ? îÒº…IUNASNone@…&_oÒóPowerLawnone?ïÿ'qÆ°˜?b%bˆ"{?£Ž$ZSƒ?b%bˆ"{?ï܋D¨aÅ?''ÚÛAPv?qº]ž­¿?''ÚÛAPv?ïߌûd²?kˆa~Æ<¹?p9¾ó/_?kˆa~Æ<¹?ïÿÿ®eGq>…fÉkkEW>"wD°Ö¼3>…fÉkkEW?ïÿ@ËÞK‹?y¬@æ|?æ‡p?T?y¬@æ|?ï"YRgè?­apöFʓ?›¿ôܒ:ö?­apöFʓ?ï´uŸX9A?'läÇϾÃ?'â˜.i-Ä?'läÇϾÃ?ïÿólìõ>ã$¥B}>Ù%ÑÒ``|>ã$¥B}AGN3FGL J1808.4-3519@vM—á2µ_ÀsV?§µ¼À9¤qJÅöðÀ;8ñ±ˆ¤?ñ/áo@
È-â¼MN@xÀ`'̤¿äñ-Çl¿á"ðŠ—=¿åp-ÇZêT¿ïýÁÜPDÞUNASNone@–2þÅm\ûPowerLawnone?Øãl[à{?Ò:w5p?ãŽIÒ1Â?Ò:w5p?À€¼[™ˆ?Å<Z¥=g?ëßÐé½?Å<Z¥=g?æh҃^Þw?±'ÈFm\+?Ó.ZùBC?±'ÈFm\+?ÕÉyÞ4ˆ?«®ä4–ŒS?åCåš=?«®ä4–ŒS?¶SØÁK"?À<ÌfAõ»?í5"çä]ì?À<ÌfAõ»?˜³Ö)ïr?³–<øƒßÉ?ï?"a¶Å?³–<øƒßÉ?Ð0ß
çå'?´ö"ªH±?ççzŒ
??´ö"ªH±? •å½Af?‹ë¶|;Ue?îö®m2*?‹ë¶|;UeMIXED3FGL J1808.4-3703@v52€ñ,(À `€ù£wÀ9ݛڼy˜À;^G;'ô;?òÁ1c$g"@Õ'X3¼@‡¿¶cÕ¿ÖáY«[Ò¨¿Ü× ÕË¿çKbã鸰¿ïÿmäñUNASNone@œò=ÈK^PowerLawnone?Ïs`³D?Í` ê
?è#;gùÓ/?Í` ê
?Ȍ¤2'g?Æ ÑÂç?éÜÏVó_f?Æ ÑÂç?áí©`X|»?³{¬<úz?Ü$­?OŠ?³{¬<úz?ۏð`Ù<O?¬||Bê·ú?â8ϓaØ?¬||Bê·ú?°'jsä?¼|ŠPa¨x?íí²±©Áì?¼|ŠPa¨x?€,?‹÷"?³¹ié}?ïþž^³?³¹ié}?ÅÊ.W+`?µÛ½jN?êtj5(?µÛ½jN?¬—š"ÞÉ?•MTœmF?î6†W{¯?•MTœmFMIXED3FGL J1809.0+3517@NýéÀ"š_@7aæÿ}úÀ:&Nw\WðÀ;¬GðY™Ï?±|a9L@
ƐÃ/@‡þ¡e–¿ä2‡»åc¿éÊ'•_!¿ÝÑnµÈ×Ó¿à¥R­29UNASNone@'|3üPHPowerLawnone?ïÿXd3õë?æ›ûÉò?óq‹4¨Ì?æ›ûÉò?ïÀYÆè(À?"Kˆ…Yó?Ó¡éÇ?"Kˆ…Yó?ïÖý:'ï?j$?»5?tbò7ÈH?j$?»5?ïáȘ‡F?T­Øt,™?n74(_rg?T­Øt,™?ïýÛÙÁ8*?8wÄÚUƒ?1!1òò@¿?8wÄÚUƒ?î2"FB¦æ?·ÞD|›Vê?¬×»˜eõ¥?·ÞD|›Vê?ïR¦æ‰6u?'l›fœn?•«#&B+k?'l›fœn?îÈ["°?•¶!*@G"?£zCÕý)	?•¶!*@G"AGN3FGL J1809.2-2725@S*I¥ÓÀ	í9SÞ¤À9X*ˆiÆmÀ:Ññd[Ê+?ìJõA` @þ~^@x›_lw"?ïÿW'rúb¿ì>Úcì¿֡Nõ¿ç[k•>.ÿUNASNone@ž…þߤ?æPowerLawnone?ïÛÀ8Gx?®¡Zÿ¼?Ÿ¤‡÷?C
?®¡Zÿ¼?é棦Éê?Ìb#tƒ?ÈeqdØX?Ìb#tƒ?í$­ðŸ?¤åû"}®?¶ß*6Š?¤åû"}®?íÎ'?z?›Ùyq­ƒ?·yŠ,)¯?›Ùyq­ƒ?ëÁÉ0œÛ?ÁMçÙ1xã?ÀøÛ?ùŒ–?ÁMçÙ1xã?ßq!h¹¢?ÓE5zqq?àGoK£}¯?ÓE5zqq?é(Ü٘?±ð'åŠ#~?˟\€™¡?±ð'åŠ#~?ç«ò{vÞ?·ŽKf=ž2?ÑШ	E?·ŽKf=ž2MIXED3FGL J1809.2-2016c@$]7qÁ
¿Óï]ŸˆÀ8)SÂóáÀ9¬†2´ˆ2?à¬Dh@
í÷ßõôc@›&@©¿ãVA`{‹¿éÞ)å¿æ"=Y|Èþ¿æÜuþ†GUNASNone@¨$ò䎊rPowerLawnone(?ÓFåö/?Ј$N
qj?æq\ñè?Ј$N
qj?îZ"€¿œÒ?º¥Ú4X;?ªVÇó*KÜ?º¥Ú4X;?Üb¦ÝhÀ"?µÐ­ìÀ²?áά'KŸï?µÐ­ìÀ²?ïÛWîÃ1?†gX¤'ä?$"ý/ö?†gX¤'ä?Àâ7œhDÒ?ÆDJóeý?ëÇråîÌ?ÆDJóeý?çˆÂdÀ?ÏÆ2p8]?ÑÆîzá6€?ÏÆ2p8]?Übª:nD?»"±¨Y%?áΪ¹bÈÞ?»"±¨Y%?ém*ǘŸ8?°©;Ð2)j?ÊKTᝃ"?°©;Ð2)jMIXED3FGL J1810.7+5335@Tq´ör2@;h}ˆÁÛÀ:|¶ýW¯À;ÞH'¶þ.?í&/Úc8_@
Ç«äÊÅa?ü{óI"¿ïþ§UCÿ3?ïôù&Ёì¿ÊÖøwG¿âOEèÂv³UNASNone@´äféxÔþPowerLawnone?ïø9†Æ6?MÕÞEjé?OæÖJ/?MÕÞEjé?îëWw
MŒ?¨ÅÇôñ?¡Jˆ'îÜ??¨ÅÇôñ?ïªt:íð<?€é8
ó"¢?…bñKc)?€é8
ó"¢?íá²É°&"?•ÿÿѝF@?°òi²~Ëk?•ÿÿѝF@?ïñ•1]£¨?\
ä¯Gxá?\՝&| ¤?\
ä¯Gxá?êTTÛÏt?Æ6šóÌ?Æ®¬Â/?Æ6šóÌ?ïE'Â"àç?"â¥T¢iƒ?—O§½[±%?"â¥T¢iƒ?èÈ=œÿ»É?¸mŽ%ˆ×?Ìß	ŒÝ?¸mŽ%ˆ×AGN3FGL J1810.8-2412@¦ÚhµÌÀ2J…_OòÀ8Œ°±
S¦À:,ñ.?õƒ-œpc•@'¡ùxƒ@—1@"ÅŸ?ïþßF]C¿èÏÊ÷›¾ž¿çHìÏ¿é/ّ×-yUNASNone@¤`ރä%¯PowerLawnone?ÐÏVDZLþ?И& T?ç˜TÝÒف?И& T?äS´Z?ÑBx'riæ?×X—J"Ò­?ÑBx'riæ?⥞EX'V?·}º½á?Ú´ÃuNûU?·}º½á?éÞÊè4öñ?¨Þ ¬Üñ?ȄÔ_,$:?¨Þ ¬Üñ?¥Æ\_S?·M
"X'?:ªÏ?·M
"X'?ÕˁÚFn5?ÑLùǛy\?å?ÜÈæ?ÑLùǛy\?Õ"y0\X	?½«ûµ²C?ånÃgÑÓû?½«ûµ²C?àeyfÔE?¼©Ÿ²?ß5
3ÖWv?¼©Ÿ²MIXED3FGL J1813.6-6845@tY+jçÕgÀ5ؖÝ&·$À:0ÅJ!ŒÀ;¸¨Uôÿ?ë@…ñh"ñ@…ÖVÍÂ@9þgú?º'¡0Dt¿ãn¤ç?ó¿íDTd ¿ßHQŸÒ:UNASNone@7~ºñPowerLawnone?ï›È.Ç,"?šG©ë'Ø?‰
ôXƒ¯
?šG©ë'Ø?ïSƒñÍÉ?¤:-?¬§ä?œuzçÞ?¤:-?¬§ä?îS'ÃÈ}n?™þHDÀ?ªÆãÃx) ?™þHDÀ?îJ+û0g?Ê"e§Õ?«]@Jct›?Ê"e§Õ?í_˜#wÔM?¹lÒè÷?µ>ãevš?¹lÒè÷?ä~? &f?ÐyM|4¯?×ف¿³4?ÐyM|4¯?é¸Ìÿfkß?²—î)Ü?ÉÌfP†?²—î)Ü?âPÙ§Ôg?ÃQ\DŠ¯­?Û^MÔ°W1?ÃQ\DŠ¯­AGN3FGL J1813.6+2820@K¡rGE8ï@4,ÙÆ°SÀ:0"t¼jÀ;¯M†›¿¬vä"`@
EiÁƒ@§†€b;	¿äj4Z`ÚÇ¿è=&ÃpX¿Ù± ˆ¿ã%ü¬,'UNASNone@ž=ø†YJõPowerLawnone?ïÿpYaú?'ÆFF'¿?qøæÌ?'ÆFF'¿?ï½ã}"S¯?"òó›üG?€‡ ¥!ò?"òó›üG?ïÝåG†Á?o0¡ËÓ»Ç?q
\U\¦?o0¡ËÓ»Ç?ï걖²ÖÏ?MŔJÅ?eNi_)?MŔJÅ?ïýRŸ›Lˆ?:Ž}'ˆ/?5kñ¾¿?:Ž}'ˆ/?î>Óx@6/?¸ïWXòÙ~?¬Èyhè?¸ïWXòÙ~?ï¤Ë%z/h?†4˜Gá…?†Í6²¢1Ì?†4˜Gá…?ï'îì‡RD?îE,)á?›"t=!p?îE,)áAGN3FGL J1814.0-1757c@)ƒÅ›€#§¿Æþ§°³'À80RÆvÀ9ŸY—K
À?íð}ø9žC@NÎLBy@s&@©?ïþ€ªú¿ã+…Æ9F¿â—y';|-¿íb=/òr4UNASNone@µžç€4mÆPowerLawnone ?¨üÅÖìéÖ?³¥Ú½ÍÁÄ?îp3¢Õé'?³¥Ú½ÍÁÄ?ê¬Ô•ª1þ?ÆÁyñ«æ?ÅL­©W8?ÆÁyñ«æ?ÖSSïÁC'?²[ü-¢†?äÖV^??²[ü-¢†?ìPyÔú!?ŸÐŠ¼n?½|1X+~ù?ŸÐŠ¼n?«IÃŐ?°hØZ¢?îOKcšr÷?°hØZ¢?â_r²,Á?Ñp@ÆTôµ?ÛA›¦}ò?Ñp@ÆTôµ?Óv#6ª¥Ê?·noOgH?æDîdª­?·noOgH?å!rÎԎã?´ìƒE6Ÿ?Õ½bVâ:?´ìƒE6ŸMIXED3FGL J1814.1-1734c@*5¤i×4/¿˜¡©¢?hÀ79™J¿@óÀ9tõɯâ?î:ÕG*ó@*bÐYÊ!@_R`u
Ä¿äüoÞùäͿ菪î^J—¿éÔnÆ $¿éK;eé#UNASNone@‰ÍèÍJ¡PowerLawnone`?¨KG^àÌc?´7W…"?î{K‰Úùz?´7W…"?ê#*f?Æ 0Þ*~j?ÅúsŸVi?Æ 0Þ*~j?ÒNG~¦?µá ¦5æ?æØÜqýÀ­?µá ¦5æ?ë—/JV¡‰?¢<lÁW?Á£BÖ¥yÞ?¢<lÁW?¶£€ä.º?ºãèŸÍL?í+ãX™?ºãèŸÍL?Ú"œOßïÈ?њêB­Ä?âî±Ø?њêB­Ä?Ô?:+ä¤?¹iÄ)Ù^?åàbê
­ñ?¹iÄ)Ù^?ÛÜq«®?µ
ÌÅ´y?âÇ*vv)?µ
ÌÅ´yMIXED3FGL J1815.1+5919@VÛ"Ðå`@; ¢G'ÝÀ:þ—J4À;Ñ-åìXƒ?î6,óå@ÃQžƒ8Y@‡ÿž[J¿å¾rMi.¿éWȄÏÄ4¿êTq£J6I¿ïý›¢ÄvÎUNASNone@€"wÎÙ‡PowerLawnone?ïº09Ðþ'?‰ÇØÖ¢7?sñÐ#v?‰ÇØÖ¢7?èzÑà¨?Őý€kAº?΀¸Á_?Őý€kAº?îÑ?(Æ?"/cÉ<Å9?¢ì
rÃç­?"/cÉ<Å9?æÄÅ`/k?¦[íÜx"?Òvu?û¡)?¦[íÜx"?ï?üµ¦H1?Ÿ"·pq?˜iDWÁà?Ÿ"·pq?Ñ·ŽþqEÏ?Ïs\\æû?ç$8€Ç]?Ïs\\æû?ëŸ-ø`ÏN?³–˜¦<†?ÁƒH|ÂÉ?³–˜¦<†?Šáš€c?¢fœŽï9?ë]G»_ç?¢fœŽï9MIXED3FGL J1816.0-6407@t¥e¶™…À4"ÕA"ÈÀ9r"#—µÀ;¤mµ@æ?æféšõ@~6QJËU@UŽ >¹Ï¿ã©WD_€n¿æX\ãZØ¿¿æÏÜ°´W$¿ïÿ:g|]kUNASNone@'ç"ÿCAžPowerLawnone?ï‡HmÏ]Ã?"Øö¹ Ä2?Ž-ä–wc)?"Øö¹ Ä2?í^™hqXˆ?³×À±5—'?µ4¼HB?³×À±5—'?ît8K èB?—ë÷ö¡P€?¨¼{C]ÆÜ?—ë÷ö¡P€?ëp*‰Ó?žþ7Ðg;?Þ?—Uض?žþ7Ðg;?íMvÕÁµd?»¾j…9^?µ"IRÎ;ß?»¾j…9^?ÚVCs?ÑB=Xlÿ?âÔÞ{öÆp?ÑB=Xlÿ?ê@8^1?´‡)óå±?Æÿ‡ï;ü?´‡)óå±?Ò|Í'‡û¯?±Q!®!?æÁ™l<)?±Q!®!MIXED3FGL J1816.2-2726@ŒS£C^À€`îWaÀ9Û6òÛÀ:òyùK?ÀõßÐyn@ý¾ž
ío@aHu«ÿ¿çv¶ÑÉó¿æÙ;®_ù¿Þ™±¾Jö¿íLøÿZ¾'UNASNone@‰"Ý—öPowerLawnone?í
616Ñ?·žÄò¼?´®OR0v?·žÄò¼?î'5o"¢—?¼q/=I%?¦Ü©±½‹?¼q/=I%?닉ÑÙÅ?©†õ9e?ÁÑظ›ðê?©†õ9e?ï™7½—¶Ò?qËLv¨ŒQ?‰² ñƒ?qËLv¨ŒQ?èatü1?É#ŽT…Ø?Îz,—;Š?É#ŽT…Ø?éØ(̎Í?Ëx†°´?ȟ\ÍDŽË?Ëx†°´?è"¼N`œ^?¶Ÿ>âþbR?ÏuÆ}Ž‡?¶Ÿ>âþbR?ìË4¬ã€÷?¦¼BÔ-?¹¦Z˜ãøI?¦¼BÔ-AGN3FGL J1816.5-1145@2}	¾º@ŽœæU4À8x‰žyÓ+À9ùÛån"B¿ðfÅê/‰0@8Lø1@Øbà¿ã¨ÝF‰¿ç¿©ò	ûµ¿émwâß¿âaÚK̘[UNASNone@Žø}¿HPowerLawnone	?Ú{ëöC"?ҙT­ßÕF?âÂ
|Þ6?ҙT­ßÕF?ï@P.¸òr?¯ó} ù0?—õú J«Ó?¯ó} ù0?àçjjà|5?·‰\‰¾'=?Þ1+*?—?·‰\‰¾'=?ïÿ?µÄêÎ?¶™öœ?	Li ?¶™öœ?Úïíûù?ЋV#¼â?âˆ9	"?ЋV#¼â?ì~
œD¸?Å¿Xɕ,?¼"EÚD?Å¿Xɕ,?âà)£'kÓ?¸Ž(	OH?Ú?¬¸Û(Z?¸Ž(	OH?ïòì'äe4?Uí]n£ªG?Z&ùс)C?Uí]n£ªGMIXED3FGL J1817.3-3033?ÿÙÞ7X\À+àÞ҈ÎÀ9ÍâÀTÀ;+	¾º?½Åƒö;±@'mÖÈ#E@v?@\¼o¿ãª"
õZ¿èStM9ſ冕l¿ããPM[Ž­UNASNone@¤€IQƒPowerLawnone?ïûFa'&#?OþÞß AZ?Bæ{4 ¹?OþÞß AZ?îͶ³Ÿ˜ü?»‹ƒ?£$"Å*‰D?»‹ƒ?ïbœOVi?'õ©ÆՕ]?"¬vJä?'õ©ÆՕ]?ïñ¸Èš`?DÍ2î£:?\Žo9¶¿v?DÍ2î£:?ïòg™fõ?oÈ<ÄÕP5?[0Íî®ö'?oÈ<ÄÕP5?ë'"‹´îN?È}¥ê'6É?Á»uÑ,FÊ?È}¥ê'6É?îùë_EF?˜^Q#qÚ? aJ	éœ?˜^Q#qÚ?ï~tà°7?'[ÝI½Pg?1cãäY?'[ÝI½PgAGN3FGL J1817.7+2530@Jh'¾‹Áj@2Ma€M˜9À9ï6¥®zÒÀ;Œo[Ømë?èä¥c§DR@•·+о@¶Ÿ¤n¿Ý3X$·Íë¿êù^QÊ¿âoµÅý®J¿ïÿµš1DUNASNone@'zö"FtPowerLawnone?ïýëò=/ò?0ü%åŽ…?0 n	N¹M?0ü%åŽ…?pà?¨ß'ÈKý'?§Uí]
ÿ?¨ß'ÈKý'?ï;®uüB?ˆpäHÞMû?˜Š?øEÆ?ˆpäHÞMû?í)ŽŸ­·?"ҝ©ñ?¶³‹	€SÅ?"ҝ©ñ?ïüÐí\©?>iŠoì­y?9x"ü×ð'?>iŠoì­y?æ"'E.?ͅÖ/ïSW?Óºûuùù£?ͅÖ/ïSW?îW§•AŒ?]( ˜l?ª…†§¤t>?]( ˜l?â!#	U¥_?¹;qþLJ?Û½¹íTµB?¹;qþLJAGN3FGL J1818.5+1320@D§¨ÖM@*|õn¬†À:&ÕÖ`ÊEÀ;Œ¥ÉRÄÉ?ëòm–¾@æÚâå@Š`@²x¿éžˆ‹v¸¿¸×mÌ ª¿â¬"ÀcT¿è'¹ø‰¿UNASNone@¥ñ»=ÈKPowerLawnone?ïÞÉÜØ]¥?vˆrMc?p›†Â©Â?vˆrMc?ì²hÙà?ÀòÅ©[ÈB?¿Úl¿é0þ?ÀòÅ©[ÈB?ïo³Cä±E?Š
D˜'­?'	—ƒi×_?Š
D˜'­?ë»(ìÍ'?ž"¹Åd÷Ç?Á\LËÏf?ž"¹Åd÷Ç?ï\¬§¤…l?–\¶ÚQƒ?"jk
' y?–\¶ÚQƒ?ÛMXªÞ\ä?ІƁá¾?âYSªÑŽ?ІƁá¾?íl]Bȟ?¬i¸þ'ú?·ÌŸà‹?¬i¸þ'ú?Û$=4úð?¶yeÄ"?âmõáe'ˆ?¶yeÄ"MIXED3FGL J1819.5-2045c@%ˊ~s£fÀ"Í*1,À8÷þ×0À:‡Û…Í3ûÀeVWz?@qÛøòÆ@¥"úI¿ço-5B¿êåCÔɤ¿àLyõܲë¿æVÈ¥1
¥UNASNone@"4!-wPowerLawnone(?ïÌ…—Gô?†ƒA¢éwÉ?yô½=úí¶?†ƒA¢éwÉ?ïyŠÖÎw?¤-»¥ãþ?Î¥%O+?¤-»¥ãþ?í´(Ön??¥FoÈ\G ?²^¿8³‹?¥FoÈ\G ?ïÿÿüÇ]Ä>aO¼p
Ø>:x­0_¬
>aO¼p
Ø?ïƒ8è?—@AsÏ¥?1ÅÛýþY?—@AsÏ¥?í;N"È¢?Âv½ºj?¶%‹cåœk?Âv½ºj?ìôл³?­Xu¸ÃõF?¿`Yz"c‹?­Xu¸ÃõF?ïÿÿq1=>£Í$]Ã*>'Ò
VÁ–
>£Í$]Ã*AGN3FGL J1819.5-1345@1mÁ¤zž?ä©À°ñÀ7éÞ(>ãkÀ9Ù)Š=D¿óÐý8zoÞ@jÔÙ`®ì@Ò$ ›«î¿ãŸ"›
jª¿ëCS‡ªó¿äêžB²¿é«F{©3UNASNone@"/ÿ|í'hPowerLawnone	?ç<ÔXv'"?ЇÀ~4ä?цWO°Ù?ЇÀ~4ä?ï>7¶O²Æ?¯¸ËVåq?˜9	4QÙK?¯¸ËVåq?átá|9êæ?¶0&ôªo?Ý=Œ*4?¶0&ôªo?ïÿÄsWï?"ŠsòÄ>ýö$î;Î?"ŠsòÄ?íþÚ³ë)"?³ø~'"Q<?°	*`¦³Þ?³ø~'"Q<?ì"ß?e?Åàï	žËn?»ßAvÙ?Åàï	žËn?è;ÊÇö	˜?²9‰ð…?ÏÔà'ٟ?²9‰ð…?ïýrz#1?1ÓÈ%ì?4l,ä8ž?1ÓÈ%ìAGN3FGL J1820.3-1529c@/Nñw§Š¿Õê'nQí3À8>ö%‹ªÄÀ9z«Yµ}ü¿ý%1¸^Ö¥@uÌKȀb@¥5À9ü¿èˆÑ§ÊVG¿é-XQ¿âA¥WÏ¿ìH	èrUïUNASNone@¯(
ÀƒoPowerLawnone0?ÉÐ,±A‰–?Ê؎Ìâ?é‹ôÓ¯›?Ê؎Ìâ?ïHÈã""?®UI$	•B?–æã å?®UI$	•B?ޔS5Ôo¦?³<.ÎWbÿ?àµÖeÈ-?³<.ÎWbÿ?ïÿá«<j{?Ü£
V=>îTåhe9?Ü£
V=?ܵDØø?Î%E¡
Æ?á¥}þ]""?Î%E¡
Æ?읎Ãt*í?Å)"M=?»‰ä^¨œ?Å)"M=?äG¤Üî­ó?´]a7Cg?×p¶F"¤?´]a7Cg?ïþàõèi?/ògþ+•?.Aó}¿È»?/ògþ+•MIXED3FGL J1820.4-3217?ç•3­ÁÀ TMryšÀ9^ê䭔À;2;Yrb?ó/ÂÖ(ì@«©Ô¥3V@À]€c½•¿Ü]©¡³Í¿ã˒ìgƒ¿æ·°ÌC¿ïÿfh¥ìõUNASNone@Ÿo~=ÁPowerLawnone?ÜaÕëâð-?Ð<¢Œv4T?áÏ
‡é?Ð<¢Œv4T?Òý6HÞ¸?ѯ!o€/T?ædې£À?ѯ!o€/T?æ©*ã^I?±94r+D?Ò­ª9ÇCm?±94r+D?á­ôæ$e?¬dÛ+GG?ܤ3·×6?¬dÛ+GG?Äid)— h?Êgä—ç	[?êå¦õšæ?Êgä—ç	[?³­A߹݉?ÆOŸ5Ëúü?íŠWÃûß?ÆOŸ5Ëúü?Ïâ!ë»ï?µ!Mƒ?èw…??µ!Mƒ?¿G?lÉÏ?ŸzAó<
§?ì¸fÆ?ŸzAó<
§MIXED3FGL J1821.6-1436c@0'j¨ëF5¿É'îz°À7ÕõŒ·_À9±Ããïÿ?ì‡õÁþ)@í{µƒ@S<À¥¢?ïõŠZCÝ¿âU¤Ÿ‡d¿âý5ò°P¿ä_æãUNASNone@¤F¬cñA PowerLawnone ?Õ딐<Åû?Î ‡Ge!ö?å
5·á?Î ‡Ge!ö?ëç¡©!eÅ?Ŕu嬹ÿ?Àay[zhì?Ŕu嬹ÿ?ÞZN††þs?¶ÕL%ÿ`?àÒؼ¼€Ç?¶ÕL%ÿ`?í'Êð 0n?—‡xò¼?³é¨lp?—‡xò¼?Ô¨Æëå/?Ì	-XÜC?嫜Š~h?Ì	-XÜC?ãÁ-+~«N?ÑN〡Í?Ø}¥©©d?ÑN〡Í?áÀÎáÇR1?·7	?Ü~b<q[ž?·7	?çqAsÍ?µ2ðê
Ô?Ñ|Åòg?µ2ðê
ÔMIXED3FGL J1821.9+6636@X"LƒfQn@;£ŒSâÖÀ:rˆšmÔðÀ<Iqc?äEO¶²ÀB@ð`™ËX@S—Á¼M¿ëóL´ÓK¿ßuÖ¤o"¿Ûô¹"'¢¿Û
`ߌUNASNone@§ðУ×
=PowerLawnone?ïþ²D‡? à·Fü¼"?$Þ¨ë]3? à·Fü¼"?–Bo?'¼Çåêý{?‡^¼,h?'¼Çåêý{?ïގ{áÖR?iÑ
,òÿø?p¸Âƒ2ú?iÑ
,òÿø?ïILœˆ.?':
"añ?ŸÖj·,G?':
"añ?ïø´F:™P?Ju•m–·i?M.æÊIµ#?Ju•m–·i?ê'Ç̀ô)?Å5Z=@ÛÆ?Å´àÉü/]?Å5Z=@ÛÆ?﷟{RS+?€2Åx½O…?'!;éU?€2Åx½O…?èu7L?¸ý [(?ϒ+#¢Ð?¸ý [(AGN3FGL J1823.2-4722@u°í(ŒçÀ.R‡;©À:И3hÀ;ŸÁ}ä1m?ô)Óݍ9@¬4VHáñ@TÿÀ,³?毐c1u¿Ìŀlßk¿áq™ô™€«¿ïÿô›.*qUNASNone@ dEzxl"PowerLawnone?ãÄÊ͐Ž?Øfmû9?ØwþjdÞã?Øfmû9?ÅA²?‹d?ȱë2q?꯿Sp'?ȱë2q?àêÇS2¤?µ"ûÈô…?Þ+ÈqYš·?µ"ûÈô…?օ×4Ú¨-?°Jˆ9âß:?ä½e'«ê?°Jˆ9âß:?Û¯Mp N?Öæ.ȕ[?â(YGïØÀ?Öæ.ȕ[?©Üà©ïZ?ºe±I?îb1õŠJ
?ºe±I?Ë&êä‡?³ó{T—?é>6yFÞ?³ó{T—?±o¬ÐÃä?›}k×Ãg?íÒ
~*Ÿ³?›}k×ÃgMIXED3FGL J1824.2-5427@uE	k¹Œ~À2
cÇOµÀ:WL0À;¯rçԐ?éƸ	µû@}ò

@¥ØߪŸü¿ãYÝUtëS?®ì:•ñý¿å8S¦ù²¿í"vmUNASNone@›V†Â&€PowerLawnone?êŒÕ•7#?¿ã*\J?ÅÌ©«#s'?¿ã*\J?íÈŚî?µˆ*ßæ?·¹¹ÑpÁ ?µˆ*ßæ?êa6ýüg?¬@Ð}üó?Æ{%Èd?¬@Ð}üó?ë—hçË?žw•X"_ý?Ãá¢\`Ô?žw•X"_ý?æc•ƒµV¹?ÇÞP>#?Ó8Ôø•R?ÇÞP>#?ڛ1:EÝ@?ÐmAKT?â²gbÝ`?ÐmAKT?å;z,ۚ?¶¯ò±(?Ոý¦HÌ?¶¯ò±(?Õó<ŠlL|?³Cü~þÿ?åaºÉÙÂ?³Cü~þÿMIXED3FGL J1824.3-0620@82Ø]ú‡@©U´g{9À8‹'®›‰^À:š'Bdÿ^¿õù}d¯­@
éGZÝq5@òø‹áu¿ë(¡–­¿áҝç˜;¿ÊwÃÛâi¿ìè2a"³UNASNone@Ÿ³gæšÔPowerLawnone?çñuƀ­d?Äó˜Ë_ܬ?Ðrþ¥7?Äó˜Ë_ܬ?ïL¬O˜ˆf?¬æ,Q9%?–jv…ù)?¬æ,Q9%?ç,`¿ø?±æ†¢À
§?Ѧå>€Ò?±æ†¢À
§?ïÿR‹ñ™?%ï``•ÿu?³óû(I?%ï``•ÿu?Ù+PÕ'?Ë":aЪ?ãjוl}?Ë":aЪ?쀫€Ä-
?ÅÔçÊif?»ú£ùޗ"?ÅÔçÊif?ç7ïw
'D?³uL¨µ?ѐ!êÛx?³uL¨µ?ïôGxv^?YÝõ'$n?Wpċ"D?YÝõ'$nMIXED3FGL J1827.6-0846@6k"Àh¡?óݑ[¶ÓÀ868À:;¾íæù?֘nyé@I—M¹ò@åÎ 3ý¿çAT惤‡¿ã²')Þu¿å·x®¬?'¿ççÁH›`UNASNone@—U­w1ÅPowerLawnone?åLÕYùo?Ðã7êŸh?ÕfUMÔ
"?Ðã7êŸh?î'dž1¦8?·ë½gNÕ?¦Ù¶yQ?·ë½gNÕ?äéËwÚy€?¹ØSžv?Ö,iK
?¹ØSžv?ïn´üˆ?x˜Ì+€Å?'>?‡¨¡?x˜Ì+€Å?ÒîÀ0Ëé'?ÏS®é7¸?戟çš7?ÏS®é7¸?èÒ¾'÷(?Ìü³(z·E?̵­¸#a?Ìü³(z·E?áAU½C9]?¼d;؍5?Ý}T…yF?¼d;؍5?ëSæøO»?§¢üŸ/—?°dÁå?§¢üŸ/—MIXED3FGL J1827.7+1141@Dd	þ†ƒ<@%	Ž«ÿÎÀ9›iK4ÄÀ;[ C×Æ%?õe3€µòì@
9r&@år?ãoÑ?î4~{ŸÍT¿áp$2íÆ ¿áOþðáT¿ïÿð	V¯©UNASNone@ž£+¹Œ~(PowerLawnone?Ã(ãP>SD?Åô©?~ð÷?ë5Ç+ðk/?Åô©?~ð÷?¸Ÿ÷vŽš?Â¥hɆá?ììfÉ|?Â¥hɆá?Ü~ë}'ü?µ1µÊ¤??áÀŠA7õ?µ1µÊ¤??Õ¤Z©U	®?®ŒS–ó$?å-Ò«U{)?®ŒS–ó$?Ÿè•8™­?°`™X¥4b?ï»V$FS?°`™X¥4b?£E¨õá?´Hn:Ã?îË¥pp.?´Hn:Ã?³æ§ŠŸ¶?¥ìG–‹ø?íƒ=E¥É?¥ìG–‹ø?³³Ð'l8>?šfO¾yåÚ?퉅íÀ7h?šfO¾yåÚPSR3FGL J1829.2+3229@NRs×Ûõ@2"Ø#B$hÀ9þJÁÅ1ÎÀ;¯Ux™]?ô)ÎØÀ ï@•kâ@H?ìT'?†F¦¿Ýl0%Ú'¿çÈRoò¿ïÿÆ:Gµ²UNASNone@'ÃìÙè>BPowerLawnone?ÙE"8äøé?Íz@9?ã]n㍃Œ?Íz@9?Ö©È@öë?Í" IrK?ä«}߄Š?Í" IrK?âòúµN'?¶&¸—ßÐÎ?ÚÞ
•bÜ?¶&¸—ßÐÎ?à£hú.H­?ª6¸¯Ñ—Ì?Þ¹.£n§?ª6¸¯Ñ—Ì?À㾸¯Uæ?Õ۞÷§l?ëÇQÔ*‡?Õ۞÷§l?¿nŸc û?ÄÜiz†M?ì=l›á?ÄÜiz†M?Çœ©)Àª?³y4–??ê?˜ÕµÖ?³y4–??»&âWc-?˜Õ«À# _?ì›#¼•š?˜Õ«À# _MIXED3FGL J1829.2+2731@Kæe+ÓÃ@0­Å÷Æu›À9lg"cϳÀ;Š¦Bˆ?ðÊÅ~#òN@'‡µÁms@õЀ5šl¿ãÇa/Åæ¿êbà[09¿è'íþÔ:¿ïýó®Á|•UNASNone@~ù›ºÜ	PowerLawnone?î}IԁÄ]?¦ÔOvU‰Ú?¨+bºwo)?¦ÔOvU‰Ú?æÊíþ'?Èäz#…'?ÒkÜ%ÊÝ?Èäz#…'?í®¤ž8? Øuvã?²úÙÄdÆ? Øuvã?æýÎÙ'µ7?£òn}ÿ7Ã?ÒbM°•'?£òn}ÿ7Ã?ë™i?¸?¿¦×Î;?z?Áš[û¥?¿¦×Î;?z?Ò| ˜?Ï_†zzfñ?æñA¯³ós?Ï_†zzfñ?æt†æR…?ºïœðçb?Óò3ÓZõ?ºïœðçb?È ÍÏp?£«p;dk?é×̌#þý?£«p;dkMIXED3FGL J1829.2-1504@1ÉêpLÀ`QyoW§À9$¤úö¬À:ºÊ9t•Ô?íE!@R¼¢@PԃÐZ?ù±Iß/¶¿ï\ ރ׿Ç2"J¹¿Þ†$æÙR¿Ì­ÞJÄUNASNone@ÒŽ"uPowerLawnone?îÖºÅÊ`G?²oýñi;?¢"S£YûŽ?²oýñi;?í«?"'äª?ÁæÚr°T?²¦Ûó²?ÁæÚr°T?î(šõ¨ýÔ?žç=2Ùx?­vP¦L	¸?žç=2Ùx?ï,ZAü

?"ù'Déþ‡?št·Â6ŒR?"ù'Déþ‡?îcå¶0\?­Ö·lY?¯¹Á¨–??­Ö·lY?ãOû©6Î?Ò×Uk0>{?Ùaà­'d?Ò×Uk0>{?ìxžˆ…?§4çª~R?¼?£»Ó‰?§4çª~R?ë.ý!1?³á"'†Òy?ÿD{;é?³á"'†ÒyAGN3FGL J1829.3-0135c@<ýæ>Ž@ÀgHäu`À8É2=jÀ:hƒwe?áŸ4eã3Á@
¨×z$ß@JMà]£I¿Ñ-ðŽHÌ¿ä¹ï[ ˜¿ãWìEÒ·¿æ¿ÿL¯c¹UNASNone@¢z¾vÈ´PowerLawnone4?ßf‡ÛÅÓ?Ó!¡2Œ'?àLö¼?Ó!¡2Œ'?î|`"?·•"°*4?¨6ÿõ²ãÜ?·•"°*4?å:ã%§?¶2^ü–'I?Պ9Í´±×?¶2^ü–'I?ï¤f|5Ü?€°³Ÿ‡v?œËs+Qڗ?€°³Ÿ‡v?Ò¾H©›«?Ï¥¹×Û?æ Ûõ+2*?Ï¥¹×Û?çÃñxl'?ο÷5oè4?Ðx&ÛÙ?ο÷5oè4?å-Q:–e?´7RÉóËâ?Õ¥]ŠÓ5Ð?´7RÉóËâ?ê™ÜÇÊ7?«Ä> µË?ś€Œà×#?«Ä> µËMIXED3FGL J1829.9-0203c@<¥£Â‡è@°ò¿-¨À8~MZü¦À9åÈÂ|ó?è˜è…K?*@©ˆGØ%@åŸ×vI?ì\±àüôL¿áJ~]ö+¿áBö\"(ç¿ìyI{…B±UNASNone@¥^"MÒñªPowerLawnone ?¡{::¼Ô?±Ð«.»€ÿ?îèL\FtP?±Ð«.»€ÿ?èVj¸Z¤ç?ʇ;½ä}?ΦU•lc?ʇ;½ä}?Ún¸´*Ù6?³Vàù|?âÈ£¥ê"e?³Vàù|?ëú´ø«ß?£èÂxj\Ü?ô,P"?£èÂxj\Ü?¤îÕZ«é?­FÎËn?ã'?­FÎËn?Ü­ÉØ·ÍÈ?Ñ»^ó!íˆ?ᩤ?Ñ»^ó!íˆ?Ü¥\H³Ö?¶Oñä¯"µ?á­QÛ¦¸?¶Oñä¯"µ?à¡¥'8²'?·»ó^ý~€?Þ¼´ûŽšý?·»ó^ý~€MIXED3FGL J1830.7-1630@/Ò¬Ùè>BÀ=Šú`"À87 ޜØéÀ:‡ºÿDï¿ÿ˜!<Ю@"ˑ¹Pn@ƒ>@'|¿éôÉwq•]¿âa¨ÀÂÂ!¿ãèH¿?#4¿è€¾­`‡UNASNone@'zµY³Ð}PowerLawnone?;$?'ST9)è? ? àÒí?'ST9)è?ïFWt¨jå?®>œe)d"?—5jò£\?®>œe)d"?쁤'ÆìŽ?©ä"ŸJü?»òÛiț?©ä"ŸJü?ïÿÜOôè>ûômƒUaü>ñÀ?‡°Ù>ûômƒUaü?íe+€ŒWg?³'V|‹V?´Ö£ùwƒM?³'V|‹V?ì~_œGÉÃ?ÄàÁ‡?¼
Á±ç?ÄàÁ‡?éŸWQS7?±Wò6ªS?Ë킢º³"?±Wò6ªS?ïüK¦U??A¨ý»ù¢?=§XÑ\™0?A¨ý»ù¢AGN3FGL J1830.8-3136@՝CrFÀ#®ç£è`À9·ÙfhÀ;TæØÍ®?ìCÓU–Ï)@
®ññÊ]1@€®_ybB¿ßu¥Ô:X¿¿³ý!£ê¿æ+x±Â…K¿ì8BáòUNASNone@š~~($xPowerLawnone?×âqY‰‰+?ÏÁéí¢è?äÇS;;j?ÏÁéí¢è?æ½åÚ–¨?ÎÄ«‹^˜g?҄4KÐÒ°?ÎÄ«‹^˜g?çt¿¬?±±ýw;U)?Ñ́ð§ë?±±ýw;U)?éZZ½6=?£¤=ªŽ.?ʖ—'?£¤=ªŽ.?ØZ_=?Æ<g¼t1x?ëéh8ùq?Æ<g¼t1x?яͮÛ0y?ÐÒEÀ‡!Ð?ç8('gÄ?ÐÒEÀ‡!Ð?ÙÅžl´?Á®9C˜†?ã}°É¥À?Á®9C˜†?Ò±fEj~Š?¯;7Âòªî?æ§LÝJÀ»?¯;7ÂòªîMIXED3FGL J1831.7-0157c@<ðÞÁÁÖÐ@źcdÀ8U["¤À9›hýð[GÀ6O†{×@
#nýcÃt@Q¿Š¿ã%ïÓ·ø¿ìxÌwí\¿áœºBÜs‰¿ã–σ$UNASNone@ ¼þ\'ÑNPowerLawnone0?؂Ѹç4$?Ñÿ¾pWoÂ?㾗#Œeî?Ñÿ¾pWoÂ?ïtŒÚÌóA?¥·Ý¼2?'nd¤©Éç?¥·Ý¼2?âÔØ?³i'r#v?ÛÁðVOÿ?³i'r#v?ïÿö-Kñ#>ëžPœtQ>Ó¤è+0Vã>ëžPœtQ?æʵ©"?Ë(bnN-?Òj•Ô¬Ù×?Ë(bnN-?íF¶°€»Ò?Á]¸ÿäã?µÊJzBSq?Á]¸ÿäã?ç'6Ê}£U?³ï×@ë˜ð?Ðû'k¹V?³ï×@ë˜ð?ïÿS–ÄÁÕ?$é¦ÙL	?!Yu ï?$é¦ÙL	MIXED3FGL J1834.8-0630c@9?î¢	ª¤?ænø`¤Z"À8í^<Ì9À9Øî
5?Ñ𢐟[6@¬fjÃl@²m?ôa¼?ë S0ºÄ¿íö:"`L¿Ô=XRHï¿ÛóÜApUNASNone@²ƒÙÀëíúPowerLawnone ?䋋wÔ<?Ðÿâ ú?ÖèéWï‰?Ðÿâ ú?î¸éôƒ}¬?·ì+gmê˜?¤q`¶ì>A?·ì+gmê˜?å°×Ôå†?³ÕÕ\ñÑ?ԞPWÜ4õ?³ÕÕ\ñÑ?ïÞÄ·],‰?^Ã+28¯o?p¤`ˆ,?^Ã+28¯o?çÕm­'"ª?ȍŠ…7?ÐU$¤úö¬?ȍŠ…7?êx*~{(?ËÉYK†ø=?ÆïVb?ËÉYK†ø=?ê70qšÖ?°§Ý¥,ã?Ç#?¾9"ª?°§Ý¥,ã?ï}×ú'xë?'4}IҒý?E¹Y©?'4}IҒýAGN3FGL J1837.3-2403@#±©É'†À<µ]D~µÀ9v"´/GÀ;}}?ÕÏ\t@9muÏ:@6tªL¿çá©	=\¿Ü,Ûàæà¿ãQG¯'[ ¿ï}§SÒ¡3UNASNone@'FsØPowerLawnone?äo.¢"â?̨—á2­?×!¢»ðö<?̨—á2­?îg]\ÙA?¶äô}—?©Š'ëRê?¶äô}—?èúY(v|ð?±¤¾0"×Å?Ì›^&??±¤¾0"×Å?îÈ}›f?…©þš…?£x&H½SË?…©þš…?ÓV¬.éð?ÍÔ=Y|Èþ?æTž©è‹?ÍÔ=Y|Èþ?æÜNÚþê?Î6b®‡"°?ÒGbàJ-?Î6b®‡"°?àðAãi
I?ÁՊx5é?Þ|9-ëm?ÁՊx5é?æû±Øq?µfÏÅ?ÒœOñÔ?µfÏÅMIXED3FGL J1837.6-0717@8ÝÔÇm{¿Ñ0‡¼øCsÀ8Y­N'DÀ9¹÷[ÐL¿ÐÈlåJ`æ@
Âp¡æð@L¶€… '¿ìpÑVýÆ¿Ìö%°,œÛ¿çÓV˂Žª¿ãËy:{žUNASNone@ÀÏ|í'hsPowerLawnone?Ý=Æô_|¬?њUÇå"?áa…ÐAª?њUÇå"?ïQwI–*?³z8¼Pò?ŸõÑîÔ?³z8¼Pò?àf'	HíÉ?¶'aÉ÷1?ß2ûín$m?¶'aÉ÷1?ïðHœžS4?W†"Ëú't?_nƆàx?W†"Ëú't?Õ[Ƌ{Z?ÌÎ݂@{_?åÒºBS?ÌÎ݂@{_?ëYëºV?È)º¿ë#5?™‹àQ§?È)º¿ë#5?äsËs}Èz?¶?‰ú?×io?¶?‰ú?ï9©žÁÃý?¶ùß|O?˜ÊÌ" u?¶ùß|OMIXED3FGL J1838.1+3827@PΚ¿3‡@2åxåÄëWÀ9Ù ~(ØÀ;˯é(¿èCc˜D@›@ññP@̾@Bo¿é‡ŸeØÄI¿å;qv¡U¿æ¹˜ÿ"žÏ¿ìÍÈl¸2UNASNone@zãšÔ,<ŸPowerLawnone?ïâEþDœ›?jzðýÉd?mºßU?jzðýÉd?ïÌڜ¡¿a?‰Çù–O?y'±ÅÍ»?‰Çù–O?ï©Toz?ýä½qt"?ŸjÕk>ØÒ?ýä½qt"?ïö—…‡Ö?A뱿¾Í'?RÐõL²?A뱿¾Í'?ïŒ>ú^!ì?Ã|²|@M?ŒðAkç!?Ã|²|@M?î§$¹¾"?³"9HÑ#?¥´oDÁ?³"9HÑ#?îg'AÐHÇ?œÜ¯"A·"?©†ÛáC¥'?œÜ¯"A·"?ï+Ó£*¼í?'xAî-£?š…‹ŸÏÌX?'xAî-£AGN3FGL J1838.9-0646@9zTæâ!É¿ÔAKdWmzÀ8:úêíIDÀ9ýèwM>?ÓS–=w7x@RQR-q?þ¿>«Œ`?îÅUÌ)'°?ëL¦*õÏ¿ßÙî7D¿åŠ¯nÍ#UNASNone@¾ðPowerLawnone?èÈ?Åpjª?̀ýt)+?Ìßê>UY?̀ýt)+?î~!,k?¶aסÂ&?¨íê«dZ?¶aסÂ&?åÔBÄÃ
y?³ñz_7`#?ÔWzvyë?³ñz_7`#?ïxöà¶R|?î—ÃÁñ?á#î]?î—ÃÁñ?èO	»?±œ?Ç¢¬—‰?ÎÃÙ9'?Ç¢¬—‰?ê	ôèõ¢Y?˞ØlW?ÇØ,\)vœ?˞ØlW?ê%=ãK¥?°N>ďP:?ÇkrÑiü?°N>ďP:?íö¦n­÷c?¥îÔÚCu#?°J̈Øvç?¥îÔÚCu#AGN3FGL J1839.9+7646@[8›R~@;ÅïbúÀ:po»y¾2À;ÿPïܹ¿Ÿ9%ÑÐá'@
˜áT@ld¿ó¿ã±Š#"ê`¿è¿|¤¶¿âܪ̃¿ï"wõºUNASNone@"ƃ{J#:PowerLawnone?ïõ—i¾‹?Rò_ˆ»£?TzÑRþŠ¡?Rò_ˆ»£?ïËΟ'3C?…ƒe/´q?z°$ÉV¬?…ƒe/´q?ï$êAõY?Œ›u•BÝ?›b·Ãâí?Œ›u•BÝ?ï'¤_+›?pÌMÅ^…#?‹}ÝæE\?pÌMÅ^…#?ïó6öX®º?Z–Ýàñöì?Y'"§‹Ô?Z–Ýàñöì?íê."b<?·_$=ºO?°®TÇ,¥?·_$=ºO?îêÚ\ˆ–?™Ÿc±?¡RZCW—?™Ÿc±?ê†3…éc†?²³Šï?Åç1èZqæ?²³ŠïAGN3FGL J1840.5+6116@VÀŸ±@8ÙìÔªàÀ9Üuι6À;›¤xð­¿èù+¥þµ[@´D¼­@۞ÿµ¿ë÷&~*8Ÿ¿æ:QB›c§¿á@Æ®-X¿ìªJkßUNASNone@€é2a|ÚPowerLawnone?ïøØäˆ*[?I"
8;H?Lœm†ÓÕá?I"
8;H?ïØöËÆ3ù?'äi…¯sÍ?s"š	KÁ?'äi…¯sÍ?ïçŒIW•?…1¢þk÷?†íª¤?…1¢þk÷?ïüp¡RË?*ÍLØ­w
?<zô3"?*ÍLØ­w
?ïô|…ñ?]¹ƒA…Þ?WõÓÜT?]¹ƒA…Þ?ï0i)dR?¯ž'ZÓY[?Ÿ™òÙ§¶?¯ž'ZÓY[?ïÜ»"{?–Âþ||?|"_öŠ¶?–Âþ||?ïÊ®3¦íâ?rB?
nþA?z¨æ2nÄ?rB?
nþAAGN3FGL J1842.2+2742@LÌݓÄn@,18yÄ<À9'íG–—‡À;|5vÚQñ?ìpRqx#Ž@
?çݟX@!¿mh¹¿ãMû
Qø¿ÖŒtšUè¿ßGDŒ¿ëÙ<\QºˆUNASNone@›îøºÇËPowerLawnone?èixGB{?Æxýç:Ðû?ÎZâ÷º?Æxýç:Ðû?èÞý>?ÆiÔ>R?̇‡¸	‹?ÆiÔ>R?ê*¨ŠÁ??®Ì¤ uæ?ÇU]טû?®Ì¤ uæ?è~<}¬ ?£:S§¶¬"?΃	O?£:S§¶¬"?ÛwHWBî"?̊§':›K?âD[Ô^ˆï?̊§':›K?ÕýÉ '>(?Ё¶£ë'?åo¶àì?Ё¶£ë'?áaè3ÊK­?ÀSo¢¾ö?Ý</˜kh¦?ÀSo¢¾ö?хDÍVœ?°œÀ—r>?ç=]ñT²?°œÀ—r>MIXED3FGL J1844.7-1224@56q¬À¦žË1ÂÀ9Lx䓓À:›¸®ã®¿ÖYIŸ}«Ÿ@­5'Þê\@9*Ÿ»Ç—¿ée÷"þW½¿è·×À⯿Դûï=ÿ¯¿áŒë¨ÛUNASNone@¤¶À[À7PowerLawnone?ïçß0ìJÛ?x¥å—å´?h ÏGï4ƒ?x¥å—å´?ïºLl•*?²¡on%a3?ˆ¶w"ÄÅ?²¡on%a3?îZ±–)f?¢Ó!ˆbzú?®šTä四?¢Ó!ˆbzú?ïþ4£(l? 3¸6.‡Â?.¬·Tú¿? 3¸6.‡Â?ïác¡~Ú?'Hßí»Ú·?ˆ‡§q?'Hßí»Ú·?ëý—"'?ÆÆÕ_|?Àõ£ýíù?ÆÆÕ_|?íqòrg•T?¦ƒ-/XË-?´plmŸ<\?¦ƒ-/XË-?ïô˜8¤ú?Ná=BðŽ$?VώZb­b?Ná=BðŽ$AGN3FGL J1845.5-2524@"á˜kœ0MÀ$(^ÃÚµÄÀ9]ÉòîÀ;*¾áQ¿?äkõö«‡G@
™•}U@N@A0ÿÒ2½¿ã©åÇù¿ç¢I-ÆaÏ¿Ö'ˆvîÀ¿îIt&(ÄÖUNASNone@'Nr° ĜPowerLawnone?êóDƄ?ÂHí=ÊT¼?Ä2ï«ôåñ?ÂHí=ÊT¼?ë½®Ðý!î?Â×É]š‡?Á	D¼xH?Â×É]š‡?êu‡ÛE?¬0þЀ
§?Åþ)à'ì?¬0þЀ
§?ìx°ÂøZ?\ŽÛ™?¼:yè=/z?\ŽÛ™?âr¶Ð¯?·Éw"ñ?Ûð'_ú£?·Éw"ñ?Þ1 Å÷ŠT?Ñó"~Êä?àç/:Ö?Ñó"~Êä?åӂüt/R?·Ç™	»e}?ÔXú¡\?·Ç™	»e}?á6¹=¡?À-¡Tè©?ݒß"½ó?À-¡Tè©MIXED3FGL J1849.5-0124c@?v«%(®¿ÍÇø<<FWÀ8Ê<ϔ'À9}⊤3Q?ñÂãoPšÍ@ÕÅ©@Dàßÿ.Ÿ¿æ•H\mÇ·¿â‹ƒ&´(¿æÌdÌL8,¿ìFeXäUNASNone@¯²ÀÞ҈ÎPowerLawnone<?d
tڟ(?rz@X»?ïëõéÈþY?rz@X»?ÙäÒ´åœÊ?ÎË
5h~?ã
–¥1›?ÎË
5h~?Îdæ×Þ=?°uP"¤®?èfÆ\Šq?°uP"¤®?å
6Tê'?¯gö Ó?Õëû"V*ü?¯gö Ó?P˜°	 {Ó?UíÍH«¿?ï÷³¨ª?UíÍH«¿?³ã
hô3?¿X¶ÇÊ%ö?탞²ª"?¿X¶ÇÊ%ö?´á°èhÏ?©*›¨C?ícÉâüRæ?©*›¨C?ȨÊþk€?¬Mϲ(ˆj?éÕûÍ@e ?¬Mϲ(ˆjMIXED3FGL J1850.5-0024@@;ò<ÈÞ+?'çT¸i"À7"ºV¨ƒÀ9¦AÂB/O?ôÇW<§Ñ@¦ûjo	£@[?²r"¿Øò‹p¿ŽS¿é™Óêè¿æ†Œµõ3¸¿çÍ`|Ü8iUNASNone@›ÔxFÜPowerLawnone?ƒò"R›¿?ÇÀ³üh¾'?ë_^ëY?ÇÀ³üh¾'?æFDڜæx?ÍY`Þ+Ú?ÓsvJÆ3?ÍY`Þ+Ú?ØÏUÂnò?·>꬞¾x?ã˜UÈö‡?·>꬞¾x?êÖÅҐ9?¢mØ#é?DŽ¤èµ¿?¢mØ#é?³Ð­ÎåÚ?¸Þ=£f±l?í…êFŸ5?¸Þ=£f±l?ў¬ûÝB?Ëæ´µ(ì2?ç0ô©'_?Ëæ´µ(ì2?Ùmäc[2ð?ºš…V/{]?ãI
ÎRfˆ?ºš…V/{]?Ý^z"Uª?µæÉ£!­¥?áP½Õ8+?µæÉ£!­¥MIXED3FGL J1852.8+0158@Alk΅3±?âЀÉ"À77ûº !ÞÀ9Ã~ü_a?òýó¦*v¡@üäõ‹C@`Пëf¿å0ù›ü!¿ê;ƒ[6)¿å²Æç'¿é¬ƒIS¹™UNASNone@‰Bš6âëPowerLawnone?¯/ãçZ=?¼T~¡4‡`?î
A³Ëì?¼T~¡4‡`?Úõ.Åv}?Î#·¹®üœ?â…@hDÁ?Î#·¹®üœ?Ó·?#Vq?¶ý9Ú£?æ$z`nTÇ?¶ý9Ú£?åh|s̉?«U~'T-?Õ/fíå?«U~'T-?¨ë§õ¦*?±Š–-&Ê\?îqE€Îا?±Š–-&Ê\?½j»ú[j#?ÄMcBñ?ìR¨€´'¼?ÄMcBñ?ÏÂàfÌW?ºÏEbŠ¹­?è{ÇæLê?ºÏEbŠ¹­?̏öé½?«Õu0çP?èü\E¿?«Õu0çPMIXED3FGL J1855.4+0454@Bá
£3v?õ¥+•°À7ÐÌ% †À9ù¡t?íZªŠF"@
:íO¤-@W— mˆÅ¿àï6ð3À¿épJÜ$â¿çNéWпèržïïUNASNone@£n.±ÄPowerLawnone?¸—Ó¸®'?Ã	fBŠ?ìíˆÄÎë?Ã	fBŠ?âÑÂp7?ÎäWå¼D?Ú\{ÕÓ'?ÎäWå¼D?ØßÅ""?·†)š™y?ãònû¶?·†)š™y?ç§ådü·?©¨0T>m?а56'?©¨0T>m?¨Cà-5?´5Ó|z}?î{ÁýeñÌ?´5Ó|z}?ėna÷0?ɋU"Òô??êÚ=$g'4?ɋU"Òô??Ô+®ö^QÖ?¶ÝÒoÙ>¼?åê("Ð×?¶ÝÒoÙ>¼?˧àâ¶÷?«¢"&zD?éÇRB ?«¢"&zDMIXED3FGL J1855.6+0753@D7Æø@B‹`òËÀ8J¡!À:^×òš¼¯?êSrBèˆ@xrÊø·6@Њ©³¿æÚ¯Nњ¿é
X<Ï`¿ãŒ˜qGã;¿ïæ_4eYÃUNASNone@"0a ÏPowerLawnone	?Òé¡ü¼?ÐvTΗò?æ‹/s¡¸?ÐvTΗò?˙B›®?̘""ÉÈ?é¯{ÙY?̘""ÉÈ?áäÄ6é?¶¿ÂƒÍÉZ?Ü6w"èÞ.?¶¿ÂƒÍÉZ?ÞxdÀžì?°ô'qú;?àÃ͟°‰ö?°ô'qú;?¿»Ø¢‡Ã?ÃT'÷7-?ì"믌?ÃT'÷7-?¯ÈŠjIl?ÂЄšâx?îwY[n™?ÂЄšâx?Ù"ÿ£'§?½Q›0ÑÔ?ãpî€.l-?½Q›0ÑÔ?±ˆËºi?—źvîOÓ?íÎÿfŸh³?—źvîOÓMIXED3FGL J1856.1-1217@6whۋ¬Àf•Ù¸éÀ8î¾c}}ÚÀ:ë´¬D—	?ë«Ë<vJW@ofw®7`@¶?wå¿åíQŠ"̉¿ë7ú&ïzn¿ã€<"Åý¦¿Óm'ÔUNASNone@‡ ¤xGPowerLawnone?ïî9·æ?^Õ$±þ{Ú?aÆHȟ'C?^Õ$±þ{Ú?îM/ý¸kÜ?¸Mßó†?«-&1E?¸Mßó†?ïEÜôjÔ?FWÁ÷ z?—Dat]KÀ?FWÁ÷ z?ïeœ<I	?z5æïsM?"Lx{'BÙ?z5æïsM?ïÀ›#¥?€©$þDo˜?²n%oI¾?€©$þDo˜?æq¡%d`?Ïޑ¹Y2?Ó¼åµ7@?Ïޑ¹Y2?ì½(`W"Î?¦ö‹ïÚ:k?º¼ýCY"?¦ö‹ïÚ:k?ì3W´¿1?¯VR@v?¾g½BZu?¯VR@vAGN3FGL J1857.0-7341@t]9–ûÀ:W/˜sÿ¬À9¦ÃhŸýÀ;¢«%³ð¿ÌÙÑò?fâ@OüÄâ@;z¿ä±ñ¿é€ê&¶v¿élᄌ8ª¿ç؆ð'M¿ïÿaXNeUNASNone@uÁ'}keªPowerLawnone?ïॽqî?r'v™ì#?oZB"Ò‰?r'v™ì#?ï¼ã·¹®ý?fÄ¿M?€Çàá?fÄ¿M?îùÁ\òÓ?®ÌßÀÄ? cïyÕ?®ÌßÀÄ?ïÀ£ü‡?g&%vŽª?®
ù¡B?g&%vŽª?ïׇOâbÙ?}T$eס?t<X­Ë²?}T$eס?íºÊ,ù!-?·Á
,í?²)®–5?·Á
,í?î
DÝ2SB?¡ùƒŒ'}ö?¯+²,ÚËà?¡ùƒŒ'}ö?ëèL¬DÛÁ?ª"cVˆð!?À^ÍNìü?ª"cVˆð!AGN3FGL J1857.8+0129c@A€jüοè	_s­øÀ8+-ß6[ÝÀ9t°/Þ?òö&Û6@
ÌûìJ£@½Óà'Q|¿b7ž¤&ƒ¿ç¡YMp™¿çÛَÀçU¿ë9ì¡î·UNASNone@°;6"uPowerLawnone8?€Fn8iÁK?'Ðy'ÿ»q?ï¾æFè¿?'Ðy'ÿ»q?ßÖGÕX?ÐCõ=.^¸?àÜ97•T?ÐCõ=.^¸?Ñ¥í‰t¢-?±è¬¥…£'?ç-	;E®é?±è¬¥…£'?æñš‰Ùˆ?­m$:"Ñ°?ÒÊìLïÈ?­m$:"Ñ°?xr¿²f	?ƒIœtJ?ïÏ€›4?ƒIœtJ?À³…€ªW?ÃƸ*ÿ2%?ëÓ;ޟÕj?ÃƸ*ÿ2%?ÂÍ5IÛ7Á?´"ê1¢ê?ëL²­‰2?´"ê1¢ê?ÒL8¹k,Z?´F'³(U?æÙã£JiÓ?´F'³(UMIXED3FGL J1857.9+7319@ZŽ4@9pJ¥?À	À:
ÍfOÀ2À;ö{í·( ¿ÚÇH¢õҙ@âÎ}Q@'R€«a¿è¢Ç:î¿ìzá%Qü«¿àj$׿ÑÏTŒ[áUNASNone@€óLcñA PowerLawnone?ïÿ‰L'Ëf?€"ÿ?
¬ç›²ô?€"ÿ?ïÚjmÔ¸?'yFèo´$?rÊÉ`ˆ`I?'yFèo´$?ï×ßÁàÏR?m'VŒÝ&??t1D'Ó?m'VŒÝ&??ïû!p_†?1a¼%¯å?C‹yⲿ*?1a¼%¯å?ïÿ!§ßFf?"Ì3Ô.yó?ÊýÚµš=?"Ì3Ô.yó?ï<0îñv?®ÙŒ›%Ø#?Ÿ¸yçI;8?®ÙŒ›%Ø#?ï‹$Sú܈?‡Ñè ­x?6êóŠn?‡Ñè ­x?ï°O¸‡?}jãËÜTÝ?ƒÿ,	
"=?}jãËÜTÝAGN3FGL J1857.9+5549@Ux+Iº@5GÎÙ‡+À9Î.ümÀ;GþœR±?Òvۆƒ0@Ñoƒñfµ@°uˆ÷5¿é]h»L¿¿íŒQ=pŠ¿Ï||àØ¿Ô¼ÊJ*_iUNASNone@s$X£/D'PowerLawnone?ïÿ$Mg;ù?"š¥ÜzPÐ?vM~½v²?"š¥ÜzPÐ?ïÉfÅÿ¨?‡¥-´^ºø?{L/Ü#?‡¥-´^ºø?ﳅбUD?…t|!';?ƒ‹ÞQxÓ?…t|!';?ïÜݖý¾?Z!«xu¦Û?q'4'(Þ?Z!«xu¦Û?ïýP£º‰?@€
QŠÕà?5zãZ¬æÍ?@€
QŠÕà?î2¸w]ã?·5fCâË?¬Ôx‹ÙœÒ?·5fCâË?ï`Ö !wc?\}ÉYœ?"å;ôñÛ¯?\}ÉYœ?ï!ã-r'?'ôù=xnl?›ÃšQ­û.?'ôù=xnlAGN3FGL J1858.0-5423@u`¢}ŠÀ6­Î|Ð57À:&:ØC""À;·¢Ëq'ú?ésÐ#eØ@
Aå·Tj@ô<ŒAí?ØU$äTÿÜ
Öfma¿é£*—b¿×ñŒÃ%ÜUNASNone@šmÈ˒:PowerLawnone?ïï3c i?h9E÷Qò?`̜ªÿŸ?h9E÷Qò?ï/ü,5èð?£Øµ]K]í?šzyBáý?£Øµ]K]í?ï0Ñâ"ç?öeìPÈ0?™åòª‰A?öeìPÈ0?Çg¼?ŽZ‰C¾¡?§Ås†ó?K?ŽZ‰C¾¡?ïhèÅ·ëÐ?˜nŸä°È?'âçE'éú?˜nŸä°È?åm¢;Ãif?Ï¢Ï@xÑ?Õ$»ˆy-5?Ï¢Ï@xÑ?í_'Ò*/?¥
j\ Y•?µój¸‰?¥
j\ Y•?äT"À?ÂÂlVs?×Ç×Wóº€?ÂÂlVsAGN3FGL J1900.3+0411c@B×u}Zž²¿³'¿ž¢(EÀ8XU±ã<{À9ÈQÎÿ¬ô?♺™Cˆk@
Â/,"[è@ÆŸŽP:¿Ñ:8¦öµ¿è"[clÑ¿æö&Ó±öæ¿àK!2߄UNASNone@¯Z*~ùÛ#PowerLawnone%?×ÃOX‹e?ÑÑ"	È´B?äXSºM?ÑÑ"	È´B?î®Ã¶3êN?¶šŸúÎ?¥ěåt?¶šŸúÎ?àòÑn"€?¶Ù™V+Dw?ÞÄ]"×?¶Ù™V+Dw?ïiDn2ÒT?{€ÜPþÁ+?'×r>Íw?{€ÜPþÁ+?ÉN–¨šà¹?ÉÌ¢¢&0?é¬ZUÙGÒ?ÉÌ¢¢&0?èñT=f_R?Ë>"Rq?Ì:¯
f'¸?Ë>"Rq?á DbÒÕr?¼¬"ÃH¿Œ?Ý¿w:ZU?¼¬"ÃH¿Œ?띖Ïmn¡?­½V>ÿXá?Á‰¤ÂJE|?­½V>ÿXáMIXED3FGL J1901.5-0126@@f…ÂL@JÀ]Ç@›Ñ'À8	ð1UãaÀ:'%ž:X?ÝÜ背'ô@fÖ
hHi@ò'ÿ¿âül`(‡¿èõÐF~êl¿æ"&Bý"¿é¢ó*ë¢6UNASNone@'Ý|£n/PowerLawnone?îFò9UÀ?±-Ž­¨%k?«Þ¨û
?±-Ž­¨%k?î_;‡É;?·&1^¼?ªG†ÞHN?·&1^¼?ëiqXæSº?°5vÀë2?ÂZ:œf±?°5vÀë2?îíÇÅ7=j?ƒ¢SĦ¢<?¡#ƒ«°B_?ƒ¢SĦ¢<?æHåՏò"?Éày|?Ón4Tà÷?Éày|?çV؟8?ÍnÑ-¦ú?ÑRNÁÙÿ?ÍnÑ-¦ú?ä—@̬t?¸·PZRµC?ÖÑ~f§Ë?¸·PZRµC?è
_ç?±ˆµÒÄ-?Ïó•¿Ö€f?±ˆµÒÄ-AGN3FGL J1902.3-3702c@v~ᛐëÀ1öwÄ\»ÃÀ9¾'²˝À;]Öì
¶?òb̓ìÜ@
ÈpëÐs @ˆ/ž‹q?ãÕG§€ÚR¿æ½@šF_,¿ç¾™è7Ñ¿ï ÖÊÛ
¶UNASNone@?‹xFÜPowerLawnone ?âÕ8+?Ÿ?ÏÃá«û
?ÚäU©€Â?ÏÃá«û
?×|¿Ñ=3?ÎÐ+À¼âä?äA {ág?ÎÐ+À¼âä?奮ÌlæÄ?³íZ2ÿÆD?Ô´¢g&2w?³íZ2ÿÆD?à¡w!R=Ã?±.­Ó½v?Þ½½["z?±.­Ó½v?ÎXmAp‡?ËGmV3''?èi䯹ãÞ?ËGmV3''?¸BÀ…Eî"?ã©ùõ5?ì÷§ïr¿?ã©ùõ5?ÚŸ¹:Á?¹ÝÕ.Xì?âü°#bŸv?¹ÝÕ.Xì?¸ìPùƒ?¡¥ÎÿSž?ìâ5·"N?¡¥ÎÿSžMIXED3FGL J1902.6+0655@D/Ù<FØ,?åԄƒEÀ8‰GnSš²À:Vgâ?âà:Üä‹Ê@áÊf–@؋Ÿ…ì¿?ïý—"ìпæHXT¼2¿âoO°0M¿¿å¦ÃQqUNASNone@¯<bÐå`BPowerLawnone?âÜ7ÿÛ=?Ôhhoç)Ö?ÚGÀI‡?Ôhhoç)Ö?íôKIˆ?Á +†8
U?·8]£ûñs?Á +†8
U?äÛYê&Ø?¶,#<5´o?ÖIMæ+²O?¶,#<5´o?íáÀ?ÜË?"[=‡WÊ-?°ñþÑuç?"[=‡WÊ-?Ý.-ƝïÑ?ÐՒ۱¹m?áhé±?ÐՒ۱¹m?ä¯|Ÿ@€?Ðs(LäW?Ö¡õÁ?Ðs(LäW?åQ#aëÄ?µ|͋,§%?Õ]¹<)Úx?µ|͋,§%?åõ$7ujÄ?µÞ÷‰ÉHÝ?Ô·'*x?µÞ÷‰ÉHÝMIXED3FGL J1903.9+0052@A'ʽf'À*ï9ßßÀ9O²G^cÀ:‡Ð|"µÝÀÙchÛ
Ó@ˆí$C@'& {±¿åšxBB+¿ïÇ>㕑!?í<F'Ej¿ãÔl~XuUNASNone@°…c•%PowerLawnone?ïä‹Ðƒ:³?{#ýedìe?kt/¡áI?{#ýedìe?ï{·4ÓO?¢­Ó£°½°?‰<Õ2?¢­Ó£°½°?î:Zl2-O?¢. RJ™?¬ZY<Ý+?¢. RJ™?ïÿÿ÷hú>"v·cí5Í>Q¬v®ªCå>"v·cí5Í?ﲪKºàÞ?Š—"(7ùä?ƒUm ^j?Š—"(7ùä?í\ØŽ
†?À‡3Û¤«ñ?µ?eGaÑ?À‡3Û¤«ñ?íí"ç5]?¤™ïú«*±?°"ØŖ‡?¤™ïú«*±?ïÿÿáïk*>ñC«ÊÇ)>nQk…›…Å>ñC«ÊÇ)AGN3FGL J1904.7-0708@<>iƒQÀÒWBÜôbÀ8'
DŒ!À:ä
ƒÁ¿ý¶3@=Ä×5›@²=@RU¿èØ(Ë{>¿ã@ãëªæý¿åø|
Ë"[¿îkìï.UNASNone@"×°‰ 'RPowerLawnone?ì>UTŠ	È?¹ËxŠ'z"?¾
U[¯±½?¹ËxŠ'z"?ïIªS®±?®3]¹?–Üʬó#à?®3]¹?éù¤§rRá?­z$z±í?Èmb6´{?­z$z±í?ïÿ·£Dé?äõq¹òI?5<FÁ#?äõq¹òI?àá™Kc?Ê¢k
¡*?Þ=øÍËi9?Ê¢k
¡*?ìò©È2Uµ?ÂA}Ÿäs?¸j±¿I9V?ÂA}Ÿäs?äâ6ĕÏ=?¸ÆM½Ñq?Ö;'vÔa…?¸ÆM½Ñq?ïøi\©½î?PŽ µvRÅ?NZŒg°†Ù?PŽ µvRÅAGN3FGL J1904.9+0818@DîE܃#6?éẃ}™À8̀eëí$À:&h!Q‰?Äw,S½d@û‰Eû7@`<`ƒxp?ìÏ7x¾ê¿î›æË{"õ¿Êï,ÀtÇ¿Ü}ìÑ
ZUNASNone@©l«]ÌcñPowerLawnone?ìnÙôAt®?ś³­Ê‡?¼‰0]ôZŽ?ś³­Ê‡?ï2aEℼ?°v›Ëâ'ç?™³×C¯ht?°v›Ëâ'ç?襃ÅûTþ?³iqMש?Íiðè¬?³iqMש?ïöëæ‡LÕ?@·" ìÿ²?R(2¡¯g?@·" ìÿ²?êN{<{J?řÎ6ž'?ÆÆ'Ø?řÎ6ž'?ì¾¹,m,?Ã8ª0½?º
6œ–›…?Ã8ª0½?êdÞËk½'?°¯[d	&á?Æl"ÒQ	ø?°¯[d	&á?ïæ@¬ †?`-Ö÷£Þ?i¿T(ø"
?`-Ö÷£ÞAGN3FGL J1908.9+1022@F©æî·?ìJ¬áõÓ×À8T=ÚV"LÀ:1@\¢?óÒ‰šs@
£'䞥@®Ñ¾¿â^ñ¥™Ø¿ç©Õ7Ä+W¿ëΐÌEò¿ßº¶L5kUNASNone@‰aà´áPowerLawnone?ÉM7KÛy?ή8À™k?鬲-9I"?ή8À™k?á)± 7DZ?ÒCïöiö‹?ݬ¿p?ÒCïöiö‹?à®Óž^`š?ºÆËŪˆn?Þ¢XÃC>Í?ºÆËŪˆn?çôK–×Gz?°`•¶Èïí?ÐhÒQq?°`•¶Èïí?¤´×2Á?µ@†n¶Å?î´¾ÒÒå?µ@†n¶Å?¾ZpÊÿ~a?Æn
B3?ì4±æ 4?Æn
B3?׿^dº>Ö?¼ßJD½c?ä PÍ¢à•?¼ßJD½c?ϤÔ^C|?¾èÿ͹?èÊèy¯!?¾èÿ͹MIXED3FGL J1911.1-5318@u{sBí»ZÀ8Jt֐›À:&ÇÚÄçÀ;¼¦Ô¿«?óŽP:U~@
hÍ°LŽy@žÙ€\¿Ó3T·xì¿èx1Ÿ+Ì.¿î~.ÔÝ¿ïþEõF'_UNASNone@‡LXy=ÙPowerLawnone?è^¡þíÜ<?Ç»¾ù`º¼?΅xH?Ç»¾ù`º¼?иa€ÕÂ?Í'Î0˜?ç£Ï8?•?Í'Î0˜?çæîÜÓ;?°?(]6ÿÖ?Ð3è"FY‰?°?(]6ÿÖ?Øð…§Qñ˜?¯'ú%'Ÿ?ㇽ,W4?¯'ú%'Ÿ?ç–~Ba`?ÌÖ"î9?ÑöÓ{=A?ÌÖ"î9?®òâ{®Î¿?À/'	,y†?îÑØ`ô?À/'	,y†?ãÝòŸ`N?¶œ¸'Ò1?ØDÁÍ?c?¶œ¸'Ò1?¢f'¦¶X?'(!­ø'?îٞݮÏê?'(!­ø'MIXED3FGL J1911.7+0307@Cº`Àœ~VG4À8ö}«ýIlÀ:·Ÿíp±¿ùMÛÅãúf@Á~Ëb@"éßW=ÿ¿å&5Bpם¿êE[–¿Úx+¸ô~¿äùõ§ÓUNASNone@t‡ü¹$PowerLawnone?ï÷|æQûm?e­6|W×?Q3ƒ†<?e­6|W×?ïW§ƒæ?ª/ãs>?•¨"‰9?ª/ãs>?ïLÆN¥Í?—½ÌK??ög;R°_?—½ÌK??ïÿêÈz">ç^ÞÜk{>å7NÃø—ò>ç^ÞÜk{?ïà‰Ú¬*ã?p—,Ìx©^?ov%ƒï¤˜?p—,Ìx©^?ììEƒ»6?Â{¬òo|B?¸×j˜KÒ?Â{¬òo|B?íí$^ë.?£Cˆ4Ax?°–Ý
^]?£Cˆ4Ax?ïþé&lÖ? õ9x™©?!m•#ŠZ? õ9x™©AGN3FGL J1912.7+4610@SJ«Š\å´@/‹ºw_²îÀ:>´~!nÀ;Öq»g¿áŸoã×o,@.ÁÕøÅy@‰àiÝ¿è#ðÿ㭞YzxJ¿äf¨6{£K¿åðËLD&KUNASNone@ؽf'|PowerLawnone?ïü2žðÔ?V§¦Ó0?>k"%õ?V§¦Ó0?ïÐücàœ…?ˆs ^ûP?wÎÕ¤?ˆs ^ûP?ï ¾#ð'Î?†÷‹ùY.?‡ÐvýÔs?†÷‹ùY.?ïù'Ò¯ù?6	†Zºþ?Iô·4d¦?6	†Zºþ?ïð3é³Ú°?fµ0v.ù?_˜,ÚCí?fµ0v.ù?îÍøŠ¯Š¶?³U"@-0?£ wT+mš?³U"@-0?î㣧
?œ'U¶Õe?¡ÅÎÂ"§?œ'U¶Õe?ïŒKzK'?ƒÔµ.?Œí!LSz?ƒÔµ.AGN3FGL J1917.1-3024@4¹£$\×À2x/øìˆÀ9MG8£µÀ;d¿1ٖà¿íž÷ì$Õ@¤[«Ltx@å6ÿñga¿çù@Éì¿âÎSEÞlÄ¿Þß4½eÀh¿ä$×3"=UNASNone@"ŽÛ¥ãSøPowerLawnone?ïõ\'jŸ~?Vd2·fÏ?UG±g:$«?Vd2·fÏ?ïé\Fõ)?20Y2‡?ˆ…¨ø'‰›?20Y2‡?ï¯KЖŽ€?'²Áqž?"-ɆJ?'²Áqž?ïþG°±A?!
²^]?+rÏ*u?!
²^]?ïʐšAŠ9?€¦Bª"?z·²ÓŒ7'?€¦Bª"?îÆVd*?º+@å®V?®SŸM-rc?º+@å®V?ï
—iyÒe?–7¾ÇÌ=ù?ž­פëR?–7¾ÇÌ=ù?ïç"Ï/}œ?bÍäÙļ?hk0É£+ü?bÍäÙļAGN3FGL J1919.0+0452@D76z—À¡±–¡À9!çû&|lÀ:½;ÇVkG¿ÆUm*QQ@2ÁÇ`&@Å'ßÂó°¿á•·*ã¿îIîª(nD¿Éy_+Mz¿åIĸ3ìUNASNone@ˆÀ·€4nPowerLawnone?ïú,Ñwà?H2@"
'¯?G¿L®•Ÿ?H2@"
'¯?ï> M8©%?¬ì÷•œ`©?˜;öR£h?¬ì÷•œ`©?ïšv8l?"Ájä'uÀ?=,²ðÀ?"Ájä'uÀ?ïõ…åÕ?CéÌ£k6-?Täóùy5›?CéÌ£k6-?ïÒR"ł?S3ãƫ?vÖµà ^ó?S3ãƫ?ìM¢È6?Äm¢á¨_?½'ïñ¿öP?Äm¢á¨_?íãÂ@ƈ?¢ÿÁçw?°áíøî?¢ÿÁçw?ïÆYß«‡ê?rd	å"	‹?|Ó=yÚû?rd	å"	‹AGN3FGL J1921.6+1934@JÝdob@'T¡B‡À9,¶5±'µÀ:©-Ú-Þ?ß6ðôfÞ@
òA›«Â'@òÛ¿®×¿ã)¯–Á¿èÚZ~%Ë¿åw‹Dl@›¿ìÌx('2ìUNASNone@'
"M;PowerLawnone?æ,EÌÏS?ÌÙ#}½?Ó§tfaçY?ÌÙ#}½?îЧˆx<°?²Æ¶ç(æ?¢õ‡{éù?²Æ¶ç(æ?è	(¤?Ç?´»29-á?ÏÛ]oƒâ?´»29-á?¡z}c?†Ÿ¨b›fß?¦ô%æ [Ë?†Ÿ¨b›fß?Ûš«VIR?Й'ûú'?âv2ªTÛW?Й'ûú'?çÀä{?Î&c¬w¯?Ñ~7	ùË?Î&c¬w¯?ã(–ár:?»<ßb]á?Ù®Ò=‹Ä?»<ßb]á?孑q	¶?³ï%ìg‹™?Ô¤Ýì"Ö?³ï%ìg‹™MIXED3FGL J1922.2+2313@L'Õ'å!W@B™ØƒºÀ:CĆ­-ËÀ;nÏM°Œû?Ý[ò¤ÍªB@4˜³•™/?ùÿTžè¸ç?ácØl"&8¿ìl‰‰3Îl?åD\Ñ<H0¿ºhkÎUNASNone@ÈÚ;dZPowerLawnone?ïþûO0Á? öÛNÍ? K
û´8? öÛNÍ?ï}´""?«ª'ú¾Ú?^éooÏq?«ª'ú¾Ú?ïӂäÔÞó?sj{¢¤at?v>'R¶Ì?sj{¢¤at?ïý!ê>*f?.²'i†?6ð°Ù5ä?.²'i†?ïýIKšÕ{?8äMû‹Ä?5µ¢xN­h?8äMû‹Ä?íÒU`jà?¿DŸ'‰B?±oÝS²Î'?¿DŸ'‰B?ï¤HŽ×Û?ƒÆ,Œµau?†íئ˜Ý;?ƒÆ,Œµau?ïý(uû?;0¾ú/?7VºõÝ5±?;0¾ú/AGN3FGL J1923.2-7452@sÿ'}keªÀ</Ý÷vÅÀ9ŽŒŸ5À;ª­œ…Ý$?Ûs!ëb90@mdÆ~)&@¿¥`w9¿äh1à«Y"¿æå"Ód—¿ÚƒKÀY>¿â®xŒ6bEUNASNone@—¼Æ
¦L0PowerLawnone?ïü̑5€?AL‹\á £?9›uyJÐ?AL‹\á £?ïºUéŸì?‰¼{…'?j¸‰·Œé?‰¼{…'?ïæ~"r§×?e¬.ÞÖÒ?ilY;?e¬.ÞÖÒ?ï§iáùS?eq,åb?†%‡pnŸg?eq,åb?ïø´Z×?Q&à7bjÍ?M.˜Ö;ü?Q&à7bjÍ?íé?|Ë5Q?¶Õ'º6£ÿ?°¶Ên|?¶Õ'º6£ÿ?ïºC˜ä›~?…ú sç#'?oÌŠo?…ú sç#'?ía¬c±çT?šûÑff)?´òœá"Þ^?šûÑff)AGN3FGL J1924.8-1034@;("ƒ‡ß]À(V*€JÀ9ÓôzùÀ;7›~v'¥?«x¥"éœ,@™Ã
+R@¾¦ ™@¿æ'H"¬:¿åÆ#aÃ¿Þ¾ø+}æ¿îÁç«lÍ*UNASNone@XkjçÕgPowerLawnone?ïáÄ*¼Â? b\á?f?ŸcÇu€ýÅ? b\á?f?ï&GLš¸S?¬#'ˆ–ME?›7i9Y²?¬#'ˆ–ME?ì'úó''?¤øò™µÕ,?»h/Ðckp?¤øò™µÕ,?]n¬A?uì²7	«?Ÿè§Ä‹¨?uì²7	«?ëùŸWt?ÁNWãÓ?Ì'¡Ê.?ÁNWãÓ?뀟Ï,'I?Ã_ŽcŽ"v?Áý€ÃM¶Ü?Ã_ŽcŽ"v?ç$ox³Åë?º›ˆýÂI?Ñ·!˜t+?º›ˆýÂI?ëçezO'?®?µ²?ÀbjöÁ¾?®?µ²AGN3FGL J1925.4+1605@IŠ3:}ª?zíݵõ'5À8	êâa‰ˆÀ:,îÉvÖ÷?™çÿûoÅ@µ…7âÅ]@À ý¿âî‹ÊŠ9¿é&¨¨L²-¿çM=«mh¿Ýü3¸ûDëUNASNone@'ÒØÇâ'APowerLawnone?ä"7Ÿv®?Òn´Ž<™8?×»ÁѤ?Òn´Ž<™8?ï[¹œ™SN?ªî_ïά?"ˆÌkÈL?ªî_ïά?ãŽAv9d?¹BשRR?Øã}6Æ?¹BשRR?ï»ß3y  ?p"œVí2'?3¡r)?p"œVí2'?ѺªU~?ÏGe2?ç"ò*Õ@º?ÏGe2?ëí'</Ü?ÃTUÍfû?ÀI÷@½?ÃTUÍfû?á…sßö 0?ºººïˆA5?Üõ@¿ ?ºººïˆA5?ì[Ǫ+À¬?­=bþPH/?½!®¡ú¢?­=bþPH/MIXED3FGL J1925.8-7826@s¾ó¶E¡ËÀ<@ýâïNÀ9¢îš|îhÀ;m溴œT¿´[jƬQ@
¯G·Ï @`aꁿê4,s,À¿äøã5U€¿á–"ö¶;¿ïÿÞ$8 UNASNone@‰AúKâPowerLawnone?ïÂQðÒTe?…È˦ÖÝ?~׍æё?…È˦ÖÝ?ï» eÀ?+¯ìV?7þ#§ê?+¯ìV?íøŒ7u&?HËÒ¥ ?°;žF¡?HËÒ¥ ?ïŠGO'Ž?t¶¹°Pmh?n,@kN.?t¶¹°Pmh?ïr§§àj?Ÿ"÷Ú}˙?'¼ë»À¯?Ÿ"÷Ú}˙?í'm¼­+-?¹q*NXÈ?³t'LÌ?¹q*NXÈ?ëó-CÚö0?©hV›e?À3Jð"'??©hV›e?êV5y½
ñ?²ó.¯Ú'w?Ƨ*È>?²ó.¯Ú'wAGN3FGL J1928.4+1838@JÓý`éNä?âz
w·Ç'À8‹iŽ9GÀ::
fðÏá?Ղë݉2™@
ÖLØ À@S%?ªá?âPîû¿èŸÛð¿è³ü"±E¿Ü3?_2âÎUNASNone@˜òÁTɅðPowerLawnone?áãhíÕ0?Óöôç>­?Ü9.$UŸÅ?Óöôç>­?ïGŸqbÌ?°qxçh?—*ôn~?°qxçh?å=ì¹k
?¸R{5^\?Õ߄&)ì?¸R{5^\?ï¯X¾þÙ?oˆ¡…¾sØ?")úÉ»Ù?oˆ¡…¾sØ?ÇzS@¢e#?Ì¡Š‹¬?ê!k/×f·?Ì¡Š‹¬?ì#çÊ\¹?ÃÉ3̈́O?¾äÁ­;?ÃÉ3̈́O?á'e͆¨s?»¼ù3÷Ã?ÜÛ4dò¯?»¼ù3÷Ã?í8߭؞p?¨,ÙÕXhu?¶9';'?¨,ÙÕXhuMIXED3FGL J1931.1+1659@JBeÛ
Ø¿è…uŠÆ—ÿÀ8›Âª4À:DÏkã}é?õekÒa^@žûo! å@üN¿ÓÀ?ßðÉæ,^¿ãÌjoEĿ麃㾛¿ïÿA¡DUNASNone@—Ž-VPowerLawnone	?šê˪&É\?¨E¤YN?ï(©¢®Éµ?¨E¤YN?ÍÊT*,Vÿ?ÉÛþ¿ŸMõ?èjõtê@?ÉÛþ¿ŸMõ?Ôè0ûö[?³[ÒÏöA?å‹ç'Òx?³[ÒÏöA?àSÁ™ÏÇ?®³ÿe?9?ßX|Ìaös?®³ÿe?9?d•¢€~X¶?s¯¥[,4?ïëj]R&Ð?s¯¥[,4?±ÔÙ´ofs?ºb@x&i?íÅdÉ-[?ºb@x&i?¬Â½bAß?¡7M«ü¿ü?î3Ô)§2"?¡7M«ü¿ü?Á§¨à€Ö?¤VK¬¿›?ë–:ÇßÊ?¤VK¬¿›MIXED3FGL J1934.2+6002@Vôå´$_[@27Mœk2À:Uî²ÑÀ;ö-±l¿Â†J~˯c@˜zãKz@nÿg(Ù¿ë³e"®£¿ÊlLJE^¿âð´ÁúG¿äKR6·)ÖUNASNone@¡9V»˜ÇãPowerLawnone?ïþÏé.N¿?!-SÛá"Þ?#lÍfK?!-SÛá"Þ?ïÍ+C"Ì?"ãÇpL?yj^dW¢?"ãÇpL?ïà1´Õ?e'‹;0Mh?oýÏ8ãÒr?e'‹;0Mh?ïÕ"ÁËçÊ?^ÕzˆH?unžø_îï?^ÕzˆH?ïúûiî0?FÐ,¸ ÁŒ?G¨•MQ?FÐ,¸ ÁŒ?îkv®] ?´ºÏ—	?©H•R—?´ºÏ—	?ï¿\"UŒú?~6X†ÓJ?€(ÚújõV?~6X†ÓJ?íiÙÄƲÆ?¥E³;ÌÌÜ?´±1ۂ7Ì?¥E³;ÌÌÜAGN3FGL J1935.2-7924c@s¬Ç£˜ À<£IàâiÀ9z¹9r•À;J›'§å?ä1äèç#@€9'ù@|#ꬿÇI(]ANª¿íOŒ³é7M¿ãÒìa›."¿Þ$Tý¢UNASNone@‰!ÝÌcñAPowerLawnone1?ïøÒªyA?Mæ‹"—?LµWÜ5¶-?Mæ‹"—?ï¤[Æò¡?"Žõ­"îÒ?†é?ì{ª?"Žõ­"îÒ?ï{î•kÙå?‡G÷½ßò?'-Uô_U?‡G÷½ßò?ï_<÷¢ ?u-7c¡—?"o½œ?u-7c¡—?ïëÞ'¦?nsolT&?d!å·æ?nsolT&?ì<ÀxÍé?Àÿò¥4¾Š?¾Yü9´?Àÿò¥4¾Š?í÷LOn ? ªM#§Ø?°E‡f›}? ªM#§Ø?ëÀ Íý?«Ðs"Í?øý~È
?«Ðs"ÍAGN3FGL J1936.6-4215@vJ¡BoçÀ9Õõ'^éšÀ::7yéÑÀ;³¢/jP×?ðº<|]@ò¨ À€@w)¿ìêz¿à
TYôh¿Õ¬¿;>Åc¿ê¦;Ë`ˆ¿ïÿ…'yåtUNASNone@'Acˆe•PowerLawnone?æIÇnû?ÌPŸà}?Ólàq"	É?ÌPŸà}?Öú÷þ:?ÐþÙög6?ä'ðâö?ÐþÙög6?èBñHF´?°@â®)U?Îô:Þçñ/?°@â®)U?ÝxŒêÅÂ?¯I³öcµa?áqC¹Š?¯I³öcµa?àayіúÈ?Чmrc?ß=\Ò
q?Чmrc?´‡éíêµ³?ÃTNcÕ?íoÂ',j?ÃTNcÕ?ßB5p5ƒV?ºÖÎr-2Ø?à^åGå>U?ºÖÎr-2Ø?§qBEFq"?""n®£0?îˆëÛtŸ(?""n®£0MIXED3FGL J1943.8+2518@NœwškP±?殧]Q"ÈÀ8ÑøAÆÀ:œÁ>#Q¿Ï…·3@
›WœŸ˜@Ó0?ß|¿ß	-#,]Š¿èwu[»e¿æN¶¶#׺¿ä‹oVÇYUNASNone@•üŸ¾vÈ´PowerLawnone	?ï=ð@o[Ø?¡ÚU¬Uó?˜A÷óÌRð?¡ÚU¬Uó?ï‹^yCI?¥;ídCŒÍ?(a¼ì+£?¥;ídCŒÍ?ì0=Iƒùí?«{Éù(w?¾~³à0œ?«{Éù(w?ïé D¾Ì?Sð†˜'ƒ	?f_à€'ìz?Sð†˜'ƒ	?åHÙVY9=?Î'º–Ù?ÕnMSM…?Î'º–Ù?폅ÂÞG°?¼âOã9˜?³ƒÑêՀ?¼âOã9˜?çºTœ†Ö?·³_©Jöû?Ñà‹VÆòT?·³_©Jöû?éf
¡?•{£CÏS3?¤'f/¹ö?•{£CÏS3AGN3FGL J1944.0-0535@@óò^VÍlÀ,u\WìÀ9ðáù"»¼À;D"uuÍâ?К"»Dua@|Eëòè@ijàֆ¿æגMŸð÷¿ìð¯fEÀ¿æI8̶b¹?ÝڜÝàŠUNASNone@™Íú¬Ùè>PowerLawnone?ïþ
\zTZ?3q'£I¸ñ?/Z6kò£h?3q'£I¸ñ?ïE\#¨Œã?°R'‹ªº÷?—T{'Í›Ÿ?°R'‹ªº÷?ï·òùÃa$?yMã©+^³?'A–¶ÚÚ?yMã©+^³?ïÿ
ê?˜Z0ƒ¹?ý·$E–¬?˜Z0ƒ¹?ïô:o<£Ê?fIý¡¸?W‹!'·+]?fIý¡¸?íEV¯!?ÀÑÝÒGyÖ?µÕOؼas?ÀÑÝÒGyÖ?îŽa£ø±ò?(»Wƒ?§å½Dé?(»Wƒ?ïõZ2"U?Y'š˜åª?UK›OÍUÝ?Y'š˜åªAGN3FGL J1944.1+3919@R^ÞÁÁÖÐ@V:ADmîÀ9Ý|š…RÀ;€½I¢¿Ã‹
¯ëëv@
,"GÓ@yğ»¿àôõG6¬¿ám5Ù¼Ûy¿ãä$3¢*¿æn`I°'òUNASNone@ x0ÿ—$tPowerLawnone?ïåÙÅûïœ?«û`|=æ?j&9ÓõÛÆ?«û`|=æ?ï²éGE©?™(DzL<?ƒ~­&³Û?™(DzL<?ïÕG	©Ìî?|˜—+¤JW?u\{+ÍZ?|˜—+¤JW?ïó§dAÚ?@ýâ§RJ?X±Û"ñ«2?@ýâ§RJ?ïð"i1z?u[ԋ‹ÐŠ?^Ù-!Y¬?u[ԋ‹ÐŠ?î€Ì/\Ó¯?µú½"$ ?§ó=	VÞ?µú½"$ ?ïo«dƒs?'.b•«¶B?'ª–ß-Œ?'.b•«¶B?ïw7›Þ?'y´©lÚ?'›ÈR?'y´©lÚAGN3FGL J1944.8+4300@S3¦µ(@"{¶NGÀ:Z©D1ˆ8À;¯¾ÌY	‡?ěáµ­E@
uËc–'t@!¿ím?ïæ"GÂP6¿Õ{è7È¿Öü}ù™Î¿æ̟m™
¨UNASNone@«è4êJŒPowerLawnone?ïý߅GcR?4WpßâŸø?1Ô¤Òý"?4WpßâŸø?ï£'ÔI1¼?šÙ±kûÚ?‡6
ãd½?šÙ±kûÚ?ïËöS¦=?wø]Û=Æ?zu"Å®Á»?wø]Û=Æ?ïÁÔPBÉ?cRŸO4¿?×áà{?cRŸO4¿?ïï"&)ì?g¥Sý$MÓ?`{Ù\ؔ?g¥Sý$MÓ?î#ã5*?€?¹žG‡c?­ÁÌ®7ï?¹žG‡c?ï~øD¹‡:?Œ~¶¬^t? ÷hÏÏ?Œ~¶¬^t?î¨ñj)Ù1?"ü´y¢`ñ?¥pé`Òé?"ü´y¢`ñAGN3FGL J1945.3+7329@Zd¾ß¤@@68üPHðÀ:4i¼\<AÀ;µò×s?ð9»þHoÛ@þ@ô'âÁ@XY …F%¿á1ÆT˿룠ÞÝE–¿âÔSÝUd¿ïÿ™`Â@5UNASNone@ˆÄŸò䎊PowerLawnone?ïÒx×Æê¤?'Sà?Ȧ?vÔ-Uì?'Sà?Ȧ?ã*¬Ëid6?Ì¢"–Ð3?Ùª¦i-7"?Ì¢"–Ð3?íOò]Í]
?¢rZhëÌ£?µ€mpþ—?¢rZhëÌ£?åNìë·YÚ?­0±A¹°Q?Õb&('LL?­0±A¹°Q?ï¼{®¢g?f‰ˆ¿¢?€áQû†-?f‰ˆ¿¢?È€žL?É9 æˆf?éýßØ~lÿ?É9 æˆf?é¢fÈHr?³I
°N?Évg´ÞÞ6?³I
°N?Æ5ä,S´Í?°o@ÿŸi?êr†ôëÍ?°o@ÿŸiMIXED3FGL J1947.4-1121@<æÀ§¨À1'äy'¼À9À=h@[:À;coF߸b?ò¼¥¸5ç@
Ê8ƒW
@9T h«:¿áã¼üS¬¿æ[Ëû
¿ãàý·©ê¿ïÿÆòmESUNASNone@•
'@·€4PowerLawnone?ëk%?!'?î3À»¶?ÂSk{ù?î3À»¶?ØçlH±']?Î;`­ƒ "?ãŒIÛ§lQ?Î;`­ƒ "?ê*÷†E:?¬9ÉŠ1?ÇT!æëÃ?¬9ÉŠ1?ãâo¼®û?¬'{ÊÕŒ?Ø; †¢	ï?¬'{ÊÕŒ?àF£Ûð_?Ò5ýÅ_'"?ßÑr¸HB?Ò5ýÅ_'"?·rwND?Ãvœ-a|?í1®Q‡?Ãvœ-a|?à+í…?¸¾fKœ2?ß©À%Ó÷?¸¾fKœ2?ʌz"/?¨ÐÔÀÍjK?êÙÜá~ô?¨ÐÔÀÍjKMIXED3FGL J1947.9-0743@@0,ÂÖ©ÅÀ0"ý*bªÀ9›A<á1ßÀ;WæáK	?ä]š@ÀgŽ¯…¿@= ˜ò¿ÅfÈ/¿éԇõ¾nÌ¿àiFî?Ó¿ïÿàí¸w"UNASNone@×~ºñPowerLawnone?ïâ'ktd£?wC(Îr?Á?mm"ütÓ?wC(Îr?Á?î[KFØà?´m؋‰ðá?ªO»LnXþ?´m؋‰ðá?í}ÆÝÓ
?£=Q†dÆo?·dÈ£t?£=Q†dÆo?îJ%… "^?ˆ&ñ¶…?«]§£c%?ˆ&ñ¶…?ï©݁%?"­¡…Û?…¹œG#?"­¡…Û?ç_˜\`[¾?Ë%§þÐï¶?Ñ@ÏG?H"?Ë%§þÐï¶?ëf²åE?¬‹/Œt<õ?Âg±4jë±?¬‹/Œt<õ?çM–K[s?³®Rëg?ÑdÓiIÏ?³®RëgAGN3FGL J1948.1-7059@tE¤Ý/ À>#óYÿO×À:8	=–c"À; ±Po"¿ùë›oÉ@›-—
H@¤è¿òsпçÞтFÊG¿èÒ=؆¿áɆµwÓ¿å"DkÐï­UNASNone@‹#˜~|âPowerLawnone?ïþðÑ8í1?ë:ÒgáÛ? òìj"\?ë:ÒgáÛ?ïÑf|«ï?Œ›ۅ?wLöL¨È1?Œ›ۅ?ïÁ9ªNP?| ±¶§å?qc<ãÁ?| ±¶§å?ïÿ²ø©>û~A´j?}:	£=>û~A´j?ïþ3æG®Q?.''Þ[¹?,Á˜ŠSü?.''Þ[¹?ï(4@h>Ç?°Ã¥üf]ü?šùwíн?°Ã¥üf]ü?ïoéœ]»"?‹¹Ä¦é?'ÌtHt?‹¹Ä¦é?ïø ŸÕf?L*€ ñ?O}Wù:?L*€ ñAGN3FGL J1949.5-1454@9¶¹ä'¼0À3v…3±tÀ9´ÒŠ{ïeÀ;n"WBÜô?óZ¥óš@s¯H'zÄ@Ž@À9–z?ç=Û­»:¿åJÁI-gå¿ægò(b0¿ïÿωþœUNASNone@·DµÜÆ?PowerLawnone?íºm#ÄÖ?»c~{AP?·ú,—½ÀM?»c~{AP?Ú0
3ˆ)?Îiî=,R¼?âçùpf;ì?Îiî=,R¼?æõÑøÓq?²±óu¶™?Ò\Yñ?²±óu¶™?ä,ngõ?«ÅÖ}>ˆì?קÓ"ý0?«ÅÖ}>ˆì?âûˆÐ&Q+?ѤÉoíp(?Úî_³]ª?ѤÉoíp(?ÃüÄð#?Ç£åá#yŠ?ëùÿNÃ÷?Ç£åá#yŠ?Õj´Æ¾b?»¦"³"?åJ¥œ ùÏ?»¦"³"?ËÙnµ" ?ª	ÊÓ$4%?é9I¤Ržø?ª	ÊÓ$4%MIXED3FGL J1949.6+2355@NXG¡A)¿ñ×Ê÷àvÎÀ9#ª¥æ¯À:€Ú†?à2»œ"àÖ@7í&ßgÚ@Z¶ 8Ò¿Ü·N´ ·
¿Ö³'|¼6¿ì"žZ@	Ó¿ß21k

UNASNone@¢£ Ä›¥ãPowerLawnone?è1òÎ5¤õ?ÒÏ~*ÛÔZ?Ï84Ç)l,?ÒÏ~*ÛÔZ?çØ?µ{ûÝö.µ?¥ÞO'?µ{ûÝö.µ?é«ð["¯?±#dŒ?ÉP?¦'­E?±#dŒ?îj]Góxw?'%,62?©Z+€Èx?'%,62?Ò­ËJÍÈ?Ñ*£}Ú2?æ©Zõ?Ñ*£}Ú2?ä¨m•ëËQ?Ñ>÷äŸôŸ?Ö¯$Ô(i^?Ñ>÷äŸôŸ?á–~?(½l?½y&Ёë±?ÜӁ®…(?½y&Ёë±?áÝ)ë?Âô…î–öý?ÜE­øåô*?Âô…î–öýMIXED3FGL J1949.7-8109@s‹ohÜÀ=ãæÄŗÀ9ÁC
›ÉöÀ;m±|å-í?ä¢X —>@VŠ16"@šwàŒGL¿Î"tŸA×Ŀ飨Dhuñ¿Ø©Ý ¿ê®iÆ~eUNASNone@"W}<64PowerLawnone?욈Ŕ|Ø?і<$^?»+¹Ó\B?і<$^?ï°1:.
?'-‡õÉ¿?ƒó +õn?'-‡õÉ¿?îÛr6J·+?—_BR,j?¢HܝèBP?—_BR,j?ïmQ•ÛY?pòWËÃãD?'UÍIÆÞÑ?pòWËÃãD?ﴛ­âÚ?"˜p'Çïí?'Ù?K@Wu?"˜p'Çïí?íÝð1gm?·7cu.­?±~ví6?·7cu.­?íŒ1-8a4?¤—°u?³žv–ªéÞ?¤—°u?í&îÞ3kV?¡ò-:'ü?¶È‰sL?¡ò-:'üAGN3FGL J1950.2+1215@IS6Þ¹^[ÀxK èBtÀ8Ù°i¿·;À;øìˆ3?õ…*ôö6©@Q¨ò'$\@à`}n¿ã
l"Y¿ç¨6©EšO¿í‰Îtäûº¿ïþfå^¶fUNASNone@M&Á½¥PowerLawnone?äguM`?ÆÁUäý´æ?×1dýA?ÆÁUäý´æ?»°ãÉNÏ,?ĉÅWÚB?ì‰ã†Ö&?ĉÅWÚB?èÉöÖáx«?¯§ÌŒZø¼?ÌØ$¤zR?¯§ÌŒZø¼?ÔÙz-4t?¨'ˆBΛ?å"BþéeÆ?¨'ˆBΛ?Å
H0R?ÃÌ©±"¸?ê½mý<3ë?ÃÌ©±"¸?˜Ž£mï ÿ?²úl»?ï;Šä¹ÂH?²úl»?ÛðÈÕAÕ?»ô»ÜÃ?â›ñ_?»ô»ÜÃ?¢Cß<‹Øƒ?†ºZæG˅?îÛÂn<8?†ºZæG˅MIXED3FGL J1951.3+6909@Y]uÍ·@4#ãŸw),À9÷Š1FÉéÀ;À´4O'å?Ôîhæ¦ñ@Òbœ­JQ@•ÀoF_¿éí$
Ú¿ëÒÑøß¿åْ 1+z¿Ý.ÚáÆUNASNone@}Ÿ"#ρPowerLawnone?ïþ䩄À'?FÏ@]tØ?!µi­½m×?FÏ@]tØ?ï˯Êø%/?"i•¸?z(…M@?"i•¸?ïÏM1ȋ?p-Ys¬Ê?xYzM®ž‹?p-Ys¬Ê?ïÊغÛwy?`É¥Çð…?z"¢•óV?`É¥Çð…?ïû‡wz'J?Ià–#¢õ¼?Aâ!߉ÖË?Ià–#¢õ¼?î6q‹Þp
?µ:'1žèÌ?¬˜ç@a1-?µ:'1žèÌ?ïc ¢6÷?©Y&Î%0?"œ[摷&?©Y&Î%0?í†_i^:?£¹ çiü¶?³Í¹¤Ü+?£¹ çiü¶AGN3FGL J1951.8-1102@=°É2
™FÀ2[Õº²À:Á!ßyÀ;eºßd?èr˜7]©@Ûï«ÉòÓ@֓À;ÄÒ?ï_»eàô;¿Üѳ¼©¿äÆ«¦j%¿Ûy%è"JóUNASNone@¦´?åÉPowerLawnone?ïöv_¾èš?W'çٔ÷?S@o~?W'çٔ÷?î³e–˜ïa?°æÛ<ûS¶?¤É¦–q	ò?°æÛ<ûS¶?ïeÂø–1ä?ŠDg%7£Ú?"G ð©_…?ŠDg%7£Ú?îå²{™?‡ ÈŽ®ìØ?¡¤Þ֖xs?‡ ÈŽ®ìØ?|ºÞ?ŒŽºì›6a?ˆÙ`ÑH~ì?ŒŽºì›6a?è¯I·ÌF?Ê/T™äÏ?ÍBÛù Îé?Ê/T™äÏ?íöHGR¶?¤Äfíaý'?°M½ÇÉ?¤Äfíaý'?éϼf€Æ?¶Ÿ‰
;o?ÈÁeüç¥?¶Ÿ‰
;oAGN3FGL J1953.3+3847@RzAc
'@~¡ÆÀ9T†È½¯À;
»3GU)?êU7°×‰û@
ë×j@zoÜÝ¿ÜòD…ëçÅ¿çÜ%ìèdó¿èz0¶èE4¿ïÿ™àóUNASNone@‹ä8 -àPowerLawnone?ìfQG'³?¾£隹?¼ÍuÃjgA?¾£隹?äö–£÷l?˺@ÇàÇ?ÖÒà¸)?˺@ÇàÇ?ê¶.Ž'?­ô{¥XbÄ?Å'Eǽ÷Ð?­ô{¥XbÄ?æe|ï>çœ?¥¨è¬+Œ?Ó5!'0Ç?¥¨è¬+Œ?äAI£"vi?Î+DmS{¹?×}l¸÷.?Î+DmS{¹?̑((_'?̝QtV?èÛµõè?̝QtV?ãZ\ïç{q?»àËÃs˜å?ÙKF 1	?»àËÃs˜å?Ã20²X
? ï\§r` ?ë3sÓiý}? ï\§r` MIXED3FGL J1953.4+7653@[LлnÖw@6ö¦ڜ™À:;[dRÀ;Èp0ꃗ¿Ð1¬¦ÍÅ×@¸1Hwh@ØÀ€
V¿å>ú߄µ\¿èUDÔxñ¿åCŸjþ&¿ÝÝ=ÄUNASNone@•éDg8PowerLawnone?ïÿCJ¾¦U?˜Ô(æ7Â?–§ô;«Ç?˜Ô(æ7Â?ïٛ¥æ??'såæk¤?s27·[´L?'såæk¤?ïÖ¾Ò|þÈ?sñ³¤Æ=#?t –Íß3é?sñ³¤Æ=#?ïûÞ'Š?*©ä
7«-?@ñ‡þ¤‡?*©ä
7«-?ïý‹¨â"<?7Hñbç¬{?3¢¸lS
è?7Hñbç¬{?ïCã´x?®ŒMˆwq÷?žœÊh¨è?®ŒMˆwq÷?ï‹æ¿"{f?‹ 'ÊÕd?PH2Z?‹ 'ÊÕd?ïÃÆU†¼•?tJ…—©‰b?~Õ*ÑÐ?tJ…—©‰bAGN3FGL J1955.7-7019@tQ!–R½À>ÓKµáÀ:p‹¨?NÊÀ;̽M#Ÿ?Æì,­Nœ@
+Š•š±@
@/p¿ãã…³¼8¿Ød™ó‡¿â1|ÇX¿á£LúôAJUNASNone@¡dÝ/ PowerLawnone?ïýõßÉ1j?'º"bp[é?0Q'UB??'º"bp[é?ïÄ
†%s'?(ôþµ¡9?}ù=
ÒâÖ?(ôþµ¡9?ïÓÿ|U¿?qóL~¸á–?vAٓ(—?qóL~¸á–?ïÌ }A&ï?\…Wá-?y¯Áx)¸-?\…Wá-?ïüÙz¸¶s?47Åh0o?94,dR'?47Åh0o?îa`!u=?µ¤ß˜¸ee?©éýæô`þ?µ¤ß˜¸ee?ï¤1C€¥?…{¶á|Qø?†ó¯&Ù£?…{¶á|Qø?íÏM-à[?›šàN[n?±…–'µ%?›šàN[nAGN3FGL J1957.9-0712@@ÿùÆ*\À2Ò^Ý)À9ÊØ>À;rȖg"¿Ð¼[\ê^%@
£prƒÖ@Åz¤6¿ã
e'ª6ö¿éÓb¾™¶Ó¿á"3©®BQ¿è‹Ãÿ/UNASNone@'ƒú)Çy§PowerLawnone?ïú³sú˜?M±sX}?E20fWÛ?M±sX}?ïfNë—à~?©³9 #?"6"ð6?©³9 #?ïÁÎ_p?x ™îŸ?sL‡é?x ™îŸ?ïë
ŒÃ>Ñ?OéW"³õ?dõs‡[?OéW"³õ?ïÙýRYFÌ?yÎåЄµW?sV×|"?yÎåЄµW?í?ê,ÈϬ?¾zAm;Jb?¶®˜Ý›¢?¾zAm;Jb?ïjqÊ?•ÓÊN	¦±?žýұƿ ?•ÓÊN	¦±?ï4mšã?ì²ãp?ŸÙrS'Ôž?ì²ãpAGN3FGL J1958.1+2436@O#´·,ÀQ½í@À9Õµ•x¢©À;[L
ÀÛ¡šÀ`@Ù2¹e¼È?úÜjŸ01v?æM"xºžC¿àƔR̚g¿³4ÊþҔž¿ÛPý~"xUNASNone@ËL÷KƧðPowerLawnone?ïý ÞÌŠ?7[ëH9(.?2ù	¡v£g?7[ëH9(.?ï¬GçJQˆ?–0"9»à?"î;*
ö?–0"9»à?ïÑl–xŸE?uÔ¥uNBz?wI´©"Ui?uÔ¥uNBz?ïÿÿÑJÏ¡>ƒø{jVÜ£>wr—툥Â>ƒø{jVÜ£?ïöûC¥Á?SQ'ÜËyd?R	y
Ð}§?SQ'ÜËyd?îVôŸéX¸?·Ì×^3,¡?ª¶"Bw?·Ì×^3,¡?ï¶'ˆsì?'&²âaÿº?'vü²É?'&²âaÿº?ïÿþ\­f>ºÝe­"r>¯ü]ȟfQ>ºÝe­"rAGN3FGL J1958.1-0243@CЀ¶sÅÀ0>h›À9‹•¢"À;Vé<o?ÇÂyë1@
O^b@ìi_À¿à—%oŒ·¿êðò	áð¿è9/B[M¿ïÿ®7¥!§UNASNone@yMšu%FPowerLawnone?ïÀ:†tßâ?‡&9gº*?â¼âlÆÑ?‡&9gº*?îÊu¨‰Ý ?²‰	«.ÕF?£X¥zÑÁú?²‰	«.ÕF?ퟢF³ºú?ŸI­¶­?³í̇éª?ŸI­¶­?î˯.½hè?…1M-'?£E
•¼†?…1M-'?îᚲ¦äc?©ä¬'o®º?¡æT×I‡Æ?©ä¬'o®º?çª:°?Ìïÿ¨}sY?Ы‹ðŸËô?Ìïÿ¨}sY?ëá§
?®"Ʊ-H³?È{³™cÙ?®"Ʊ-H³?ä`š6Íq?¶5ôÃ0ÍÅ?×>˒eå?¶5ôÃ0ÍÅAGN3FGL J1958.2-1413@;LŽÞT´À5§ÞÖºŒÀ9Õ¤9/ÌvÀ;t_˜?õ#¡Å¸@Ä
Ò¦€ˆ@Q%¿'6|¿ÀÈk%^¿ê!ÁduÍ¿íi=®ŒDò¿¨ÃG.ÇUNASNone@‹Œï~=ÁPowerLawnone?çh´‹…?Ò4‹øÇ&›?Ñ/ïè–èö?Ò4‹øÇ&›?欈ip†ü?Ò^I¬œU·?Ò¦ï-ò	?Ò^I¬œU·?êì'a¹Oå?ªYϤƒÞ?ÄM¶yÀm?ªYϤƒÞ?닖U[@?°Î÷(eÛÄ?ÁѦª'ÿæ?°Î÷(eÛÄ?ÚØP·[)$?Ó[–ñ|7?â"פRkn?Ó[–ñ|7?˓Îb'á?ÐÊxž:¥?ég[G¾?ÐÊxž:¥?æê4€3?³ß+Áß9à?Ò+–ÿõ›?³ß+Áß9à?Ù‰5YO?̈́Q'u¼M?ãv;eS8Y?̈́Q'u¼MMIXED3FGL J1958.6+3844@R™é9êÝY@hg~"Z•À9XÓÍ$áÀ:ﺽ֏Ä?ÚlƒÁH¾@ÉQàd)@PŸGƒ¿é×*'EÑ,¿èZAâÎkÞ¿åþ	WŽÿ"¿ì+€áUNASNone@‰˜?'æGPowerLawnone?ïè†ð'M?jP¥éøQ?gyé0 |?jP¥éøQ?ïž.—u°?•ýú]°‰?ˆtZ""ÜI?•ýú]°‰?îîõoòðè?•äb_?¡©ˆ¿ƒ?•äb_?ï®>~F?d@»€Ïì8?"p`YîÉ ?d@»€Ïì8?ï»ßû¹Ûj?…À֊ÀØ?ɨ?…À֊ÀØ?í§‹Ÿ¨I?ºè×s³š»?²Ç[¥(6?ºè×s³š»?í(T<j?¨1-
Úa{?¶½_Ô²?¨1-
Úa{?팈ЄÎm?œz:]èÌ.?³›¹{ٌ›?œz:]èÌ.AGN3FGL J2004.4+3338@Qªõs}¦?ò÷; ¿þˆÀ7Þ@c^JÀ:›ò¼K?óp"£¶S@WÉy[5±@^Ø_ýì¿àáÐûø¿æ]ª8*òP¿äË4àÝP¿åiÀBеUNASNone@'x†YJõPowerLawnone?î'Ñ͊?±'v\¤P?¯­'äß-Ç?±'v\¤P?ß4)ý]ß?Î.Q¢	)Ê?àeësÑ?Î.Q¢	)Ê?éVá¹æ?±`_·Ü¶á?ʧ""yg?±`_·Ü¶á?ä¸È‡Tó?ª=ÜûSÙ?֎nñWú?ª=ÜûSÙ?á;–—í®*?ÐCûú¯+?݈ÒÐ$£¬?ÐCûú¯+?ÀCµrŠ?Ä$àüa:?ëï¹ã]?Ä$àüa:?âQ~l{"?¸û,"Ès?Û]'õø?¸û,"Ès?Æò	8™?ªl[>‡R¯?êC}¹qÙÀ?ªl[>‡R¯MIXED3FGL J2005.7-8241@smÝ/Ÿ¾À=:úÖËSPÀ9ë:жfYÀ;‰$Ų&?Ï­¥EýÄ@ُöÏc@p0`E)¿ç"A¢¿é¶ÔÕ|@:¿â»|y(¿ïÿ­½Æ}0UNASNone@€I¼j~ùÛPowerLawnone?ïþ@éòÁ?/à:j
ÍÝ?+ñsÆYiË?/à:j
ÍÝ?ïÃÎG1~?þ"³a?~Ütÿi)?þ"³a?ï–ý5Ül
?âè­R?Š@²ŒT˜¦?âè­R?ïÁF"ñi?aȁuuÌÛ?\îy
.?aȁuuÌÛ?ïÿ9cxô?#¥°è@Q¤?ӝ8W'™?#¥°è@Q¤?î« ˆ>[
?²ìQ±gZq?¥M÷}Ò,?²ìQ±gZq?ï€ùÆf<†?+/IÃÎ?ÁŽiàzq?+/IÃÎ?íö¿Ì«Œ-?œi¶r͐?°J›íy?œi¶r͐AGN3FGL J2006.5-0939@@Q'>EÀ5‹&9O­À:˜._ŽÜÀ;¥1}PŽ?ï™ÿ¤ª2³@õæÌ}G@~Ûÿo·H¿ÜBÈÍ
åF¿éC¥×?—p¿ïþOÃ%ã?ïͦ¦óIcUNASNone@‰ù^J82PowerLawnone?ïß	Ås®?'"-èH»Ê?p{-V?'"-èH»Ê?ï>¢›Ã7?°€{¢"á?˜=k¯÷5?°€{¢"á?î$-¯Í}?Eß@Â?­½%"Œ-?Eß@Â?ïï®VŸk?c4öÚÏÞ?`Qâ®ßô–?c4öÚÏÞ?îØÊ,<&ª?±´ìV6
?¢s]<=•Y?±´ìV6
?ê™l×*?̀J¢)yæ?ŚL£Wï'?̀J¢)yæ?éøzùµ'?±ƒkœ}œ?ÈŽ+d?±ƒkœ}œ?îDÓâžMç?·Î Ò^?«²ÁÖ!'?·Î Ò^AGN3FGL J2006.6+0150@E¸²•éá±À/aǛ4¤À:3ùJYQÀ;›zé¯?ðÝ ,e@:%Ïrn‡?ýô€kJQ¿ãÉÁb"ü?ïÍØWiJ¿á`pX
a¿çµ>LòUNASNone@«½µÜÆ?PowerLawnone?ï^Öל!?£šý­ücO?"%%!¤Iß?£šý­ücO?Õý©ÛÓrP?Ñ;W"(ø?å+FØ?Ñ;W"(ø?îÒ¤uÔù?—=ÖòŒò9?¢Õ¸²"Lg?—=ÖòŒò9?⢅ø8G?´9šO}êÝ?Ú»üôs?´9šO}êÝ?írgªÍã<?º×4LìJt?´lªÚÀž?º×4LìJt?»u™3jˆ?Ä+:¼ä?ì'LÝ9'¯?Ä+:¼ä?ê;ûdŠ>?µP<¶Q§?Ço¡×?µP<¶Q§?ňµ‹,?±§ùA•Ž­?ê¸]þҝ5?±§ùA•Ž­MIXED3FGL J2009.2-1458@;³íÇïzÀ7Ôé8yÄÀ9¢eYöì[À;d¸€åm®?ñK×+Ë_å@i›ô<ÓE@' ¦Ô¿å|!SŒÄõ¿ë¹©#Ð>Ç¿éŠp|h¿î¨#§Ù›UNASNone@€Ê"aùðPowerLawnone?ç0ÒMjA?ËhҘNüù?ў[e+}Ý?ËhҘNüù?ÐÂ*Ú­?ÌуspÉ?çžê'õ)|?ÌуspÉ?ê«úKE	?ªzUU£É¿?ÅPöÒëÜ?ªzUU£É¿?ß2òc½È+?°q;&.®?àf†Î!ë?°q;&.®?å»|·¸?Ï9qSå—?ԉÏbð?Ï9qSå—?°$d'•ˆ,?Âo·Õ¼,
?íûsm­Nû?Âo·Õ¼,
?å
W1Ú?·xJï†mê?ÕåÇýQœL?·xJï†mê?°Î›_똭?—Ô‡ š?íæ,"Ë"+?—Ô‡ šMIXED3FGL J2010.0-2120@5Fw_²íþÀ:f	EùßUÀ:.P‹2ΉÀ;¤#ìnS?ñŠ¢`<«­@
[ûÈ7ç£@l€xá=?ïü[J ¿¹i8þ6AÕ¿àÊÂè-·"¿ì¿.Äí
UNASNone@¡w_|í'hPowerLawnone?Ù¸­]¾?ÐÃf 	N¢?ã#õ)Q ô?ÐÃf 	N¢?á35žóK?ЍHäpF?ݙõ"Âk?ЍHäpF?ä7ê¼e»5?´ßF;†Ÿ?א*‡4‰—?´ßF;†Ÿ?å²®).Þ¡?­"±=É:ü?Ԛ£­¢B¾?­"±=É:ü?Ò}+FL7?м'yâ£?æÁj\Ùä|?м'yâ£?ÓxŸ¡ÎúØ?Ñ´u_tüú?æC°/'"?Ñ´u_tüú?Ó\:€%÷ƒ?Á,R™Tû/?æQâ¿í??Á,R™Tû/?Ó[«f9‰¨?´®FNîЃ?æR*Lã;,?´®FNîЃMIXED3FGL J2011.1+4203@SŸ …±…I@_î} ½À9?Ú{9À:ÈTà,%"?õa
1@ë@
²ká$ž@I« §U¿æŽXõÜÝÞ¿ê÷å#¿æøá–ïi¿ÝÃëfjUNASNone@¸ÅoPowerLawnone?îÐhsíõ?²"Žb›æ?¯âùw	R¸?²"Žb›æ?åú%$¸"?Ñ1TY|?Դ嶎Ù?Ñ1TY|?ìƒ&™$‡Q?¥ê˜Ã8'?»æË6ÛÅt?¥ê˜Ã8'?ê~ˍ¹?«´,ië?ÇÆÑËå?«´,ië?ëMd,?Âxe†u?ÊÊo‹Q?Âxe†u?ËiÊ
Çü{?ÎbfMM!?é%}Ná?ÎbfMM!?é-RQ96?°iHH74?Ë¿J¶»'?°iHH74?×ÄÌãô?Â#k4VsÕ?䙎1±?Â#k4VsÕMIXED3FGL J2014.5+5246@Uøígwž@#Ìó˜éprÀ:3o­7PÀ;k¹Ù&w?íRŒ#†º;@#¶XzÀ@bÿèƒ¿éõ'–âd¿ïÿžæWê?ïúu7B?¿Üº ÆUNASNone@—Ï'†Â&PowerLawnone?ïýUHåT·?Iîø½¥-¸?5U·¸"F[?Iîø½¥-¸?ï£þ½4ÔH?"$_è‰?‡P¶:‰ö?"$_è‰?ï»u''ô?}&"ئ!£?"»¨J?}&"ئ!£?ïè(C§/ë?eç§f_Î?g×¼Vôî?eç§f_Î?ïýwóè«·?;¡¬è±au?4@b/^N›?;¡¬è±au?î
-*¶H?¼'Èúbå±?¯--] æ?¼'Èúbå±?ï€à˜º?•×_äfñ?Ÿ~ï夶¸?•×_äfñ?ïæÚœ?{f÷ƒ¤?i%ôçä!s?{f÷ƒ¤AGN3FGL J2015.3-1431@<ÎdÜY2À9oç¨mÀ:­{έxÀ;µ}Ëùï?ÊÈ­Ì_N@úٝj´?üSQ@g<?Æ]E¶©•?Èk"…þŠ¿Þ{V¦-¿ 2
W!<UNASNone@¸¢ÛdZ¬PowerLawnone?ïþú$žÆ?*›âÚ{µ"?/p[æ2?*›âÚ{µ"?ï"E|Ù<?¤!ŸÂ:"?Žà.«"ø?¤!ŸÂ:"?ï¾Sôã†?y	Ë'»?€kɆ5Ø?y	Ë'»?ïò–íº$¡?F·œƒ²Ú?ZÒ$î«}Ÿ?F·œƒ²Ú?ïø§­>Î-?L÷V´OÒ?MaKXWdd?L÷V´OÒ?íÜR—¸ª?»¦Žõ{™?±kB¨¢õ?»¦Žõ{™?ïkU讙u?‹CË;:.H?'•BëäŸd?‹CË;:.H?ï¡ÞŠô?€mGãU?‡ˆqÎo&?€mGãUAGN3FGL J2018.6+4213@SÙÆ*\}@>"ՔÀ8wöº «À:€
è j?ñŽÑä›@¨RÙÛ_@&«ÿÍ«¿Í¡Bt2œ¿ëAlKO+.¿ÜáÑÁŠú¿ì
2ŽÈìUNASNone@»,‹C•PowerLawnone?Ö'ŠÂ^?ËoúNe=Ç?äì~r:žÑ?ËoúNe=Ç?×)¼×¿Î?ÍJbF=ži?äkq¡" ?ÍJbF=ži?â#³sõì?¶_ü–0[ý?Û¸™þ)?¶_ü–0[ý?âµçöýU‰?ªŠuO½v{?ڔ0Tí?ªŠuO½v{?µ|/Ÿö¤?¾ó·áòè"?íPzþB¼?¾ó·áòè"?¸-dÇgΔ?Á%ü¿ò…?ìúSgIÿí?Á%ü¿ò…?ÓW¸åJƒ?¸Ï͆é»0?æTt£Z¾?¸Ï͆é»0?ÅlùˆA­t?©‹k(y
6?ê¤Áï"£?©‹k(y
6MIXED3FGL J2022.2-7220@t%VÿÁßÀ@LOô4ãÀ:¨t"ÅÀ<ÖÝÇÆÔ?ñ®hk#d‰@
>§3á?ÿ0Ñ@úÇ?䶄OÊ1?Á¿œS™k]?Ö(f")_l¿ìÞß}Ú UNASNone@ªÝÅF
¦LPowerLawnone?Ó
Y†jN?Ώ¾‰`"?æzÓ<ÊØù?Ώ¾‰`"?è½¾$ñÛ?˚EÂh+?Í•l8–?˚EÂh+?äÑqZÇ]?²™d«*…?Ö]JqEñ?²™d«*…?êÆ<aÛ?±ÕÌC~ø?Äç{‡¤"?±ÕÌC~ø?Ôè×Ö|?Йæ'Ö?åõù‹"Â?Йæ'Ö?ãÍÊÄðñ€?Ò<2vÛå«?Ødjvÿ?Ò<2vÛå«?ßèü¯NÈÌ?»‡‡ë"¯?à¨X›š?»‡‡ë"¯?èF9òXç<?Ça¿¸'-?Îç6œc?Ça¿¸'-MIXED3FGL J2024.6+0309@Gzš€If{À3%oü^À9ûUê`oÀ;€.ÓR"?ëhSÃ÷f(@"ŠÝ"T?þŸ`A^D?âa6FÒ¿Ó}Ìyjп×ÛÞéëý¦¿ì¦˜	UNASNone@§1¯hیPowerLawnone?é0õ×:Â|?Å
NÃßä?Ë<(£ö?Å
NÃßä?î7«L–Óä?³-Q»Â5?¬…K:]½?³-Q»Â5?çYãÉò?±xÉVÀk?ÑL8löÅ?±xÉVÀk?íåîW¬˜?^¡àŠÐÆ?°ÐŒ°ŽÁ?^¡àŠÐÆ?㾫ůç?Ê	®-ó?؃ú¨t 2?Ê	®-ó?èäÙ]ÿ»?Ê»%tG"?Ϭlšˆ?Ê»%tG"?äíHmW?¾v7GrŽ?×üà%o%R?¾v7GrŽ?ésª
™Ñ?±>ŽK=Þ5?Ëþ1W՘½?±>ŽK=Þ5AGN3FGL J2024.8-2331@4=Ž§ÎÃÀ>\ÜY1ÊÀ:'ý«'é¢À;̝{¦iŒ?é;H›¹|@
ßþWß:?ÿ2¼À»Ÿ?ïø̵O؅?ÚQY1¨!¿ÑçD6"¿ëŒÇÓá
"UNASNone@¥Z^5?}PowerLawnone?ïI·ú¶G®?—ãA^°¤?–É®^t@?—ãA^°¤?íÄ\öB?¾Ä­üI‰ƒ?·¡ÝZo?¾Ä­üI‰ƒ?뢥-ÃÔù?ª:ð´ç'?ÁukHð¬?ª:ð´ç'?ì"ÜOe‡³? ;"0«ø?»a"ÓÂh? ;"0«ø?îOv<iµ?­aŸÎ¯(Œ?«œ9d®3?­aŸÎ¯(Œ?é$Û
¤¥´?Êþ£`º!q?Ël"Émi1?Êþ£`º!q?ëœi¢Ûâ"?«Æ`kãns?ÁŽYtu¯?«Æ`kãns?çVc¹ã¼?¼NÑß±+?Ñ×S8Œ8ˆ?¼NÑß±+AGN3FGL J2025.1-2858@,Y'fw-^À@"Ý—ö+À:TŠBäÀ;°®Xm_?ÒÓ¥ˆT½@ñ8Hñ¶@}ûŸž¿è…¶ˆ×n¿äÍD¢úÊ¿Ü?Géxª¿ÕvØiþ»UNASNone@¡"Éã½PowerLawnone?ïÿKGÉe?ãÅ}]?ö–è
d?ãÅ}]?ﺢª=‰?"ò:¡dßÁ?WxI3²?"ò:¡dßÁ?ïÒFœª?t8Ë*ç±?vܱëû´<?t8Ë*ç±?ïÙ!Òã'?\üÌû	
í?s}oü?\üÌû	
í?ïþ~ÅÚÑ?&úEô8Må?(w²v>m?&úEô8Må?î\ÍêjRÀ?³u™'¥Ä?ª3!Z6ºú?³u™'¥Ä?ïØãäôê?‡ü·­r?Œ	ÇS)o?‡ü·­r?î¶q`ëRI?—'›Žì`t?¤˜éñJÛp?—'›Žì`tAGN3FGL J2026.3+1430@L¡WÞ
fñÀ*àÔº××ÃÀ9΃&À;˜(ßó?çN	÷^@ËoT¡˜@E¨@P}¿Ê/àýJ1ì¿än¸oüõ¿×û'hZK¿íi$;!GUNASNone@š"ƒ•%PowerLawnone?ï+eËáÀ?ŸwüAس"?šœFƒÇö?ŸwüAس"?îN
Çoã?²ýMυ?«^ðõLÓ?²ýMυ?ì&VÉDò?¨,Ó_Ènm?¾ÍOqµØr?¨,Ó_Ènm?íôOncq%?‹[s7<ÿ¦?°]"RjY?‹[s7<ÿ¦?ì¬xÞ'?»<§]
¤?¿Jœ9Çø?»<§]
¤?æ?ù7Ô?Ì©ôýåÀÜ?ӀåÁY?Ì©ôýåÀÜ?ée'Üqc"?±³È-¦e?ÊiôŽ:sw?±³È-¦e?æììà=—æ?µÓ|
s"R?Ò&&?"Ð4?µÓ|
s"RAGN3FGL J2026.4+4709@U-Œ*EN@ÓáF×UÀ9rÀdß}©À:ùbLLà¿å|°R
 @ù|ÙŒ@|Þ 3玿â,»ç‹Y¿åƒ‹Ç·}¿í87V¯¿ '÷Ö:ߥUNASNone@ˆo3ÀÁüPowerLawnone?ïù'®`˜?U)—?I¹F¡£Z ?U)—?ï¾1ãk¹{?''Š_IN™?€s‡+ðÙ"?''Š_IN™?ï~6øË¿?"D¡<³6?œ°9$V$?"D¡<³6?ïÿ€Ûª¾?ç­¢þ´D?Éï6^?ç­¢þ´D?ï´a
?Ž%N Òæö?'ç¾ÿ{i?Ž%N Òæö?îÀº|µ¡?³ó·Q5]Í?£ôX6_Óô?³ó·Q5]Í?ìü9" r?¬·™¿ò-`?¸7ÛÈïò?¬·™¿ò-`?ïôŽüBíL?WcÚñÐ¹?Vâ'dx—?WcÚñÐ¹AGN3FGL J2028.5+4040c@SËà"&þ?ò[·¶»À8ÑhÉíõ<À:O¶1ÔÌ?ôù`[µ]o@š
Wǽ@р:ÍÜ¿ÒÅÈ*j{Ž¿á†qŌ‰¿ë_=ú"¿ä~÷õ·UNASNone@¬žfffffPowerLawnone4?ÙË Ô?Õ<" M¨?ã/•ˆ¬¦?Õ<" M¨?çÉTí9¡.?ʒdN¼¯&?ÐmV%Œ½¤?ʒdN¼¯&?ä.òSI?¸9Ãç"% ?×¢ËYýo?¸9Ãç"% ?é{ʺh?¨B0jð¨Ž?˚€Õa?¨B0jð¨Ž?²,Éëÿ"Œ?¼éGú?íºf›ŠN?¼éGú?ÎÜ'™Þ??ʆ®½9©;?èHöˆxp?ʆ®½9©;?Ý£²\´?ºÑ-|ƒ?á.&Ñ¥ú?ºÑ-|ƒ?ÔqŸþÑÆ?¼{™d¦®ç?åÇ0~€—?¼{™d¦®çMIXED3FGL J2028.7+1012@JëÍþûôÀ0Cý?[_¢À:ˆabñgÀ;vJt˜XQÀÎރ®uÊ@ËFºÏt@ ¨?ϣ¿èº"Ÿ"€Å¿èÀží°6¿åâ'ó~¬¿Û†u¾%ȚUNASNone@"X'u%FPowerLawnone?ïðOhˆÆ?¡Lõ¿ôÇõ?_a/P=Å´?¡Lõ¿ôÇõ?ú`"?œêu®_?ˆ~ó©o?œêu®_?ïFãé–S‹?'"¨Ü8Ÿ?—#'ÆVV?'"¨Ü8Ÿ?ïÿôk>ØS7¹´ î>×'ÆN$ê>ØS7¹´ î?ïà|s‡ÐÞ?|ÎÖ ¶Èl?oƒŒ›ë¶?|ÎÖ ¶Èl?í÷#"üô)?º–`ñî?°FãV`¸?º–`ñî?íæ‡?ò*Í?£"+aõÁÍ?°ËÆܝ?£"+aõÁÍ?ïþ
Bñd?4ü$œ‡¾??/Ï_RZF?4ü$œ‡¾?AGN3FGL J2029.5-4232@ve†á›ëÀA¾^9q;À9Ö-Š|Æ$À;±+hc–¨?îsÛïÕe@
|+Þ«¢@öã•Ò¿åæɕµ´W¿äd"p 4º¿ídÓÈÙ<¿ïþ†ìwUNASNone@"RQ¢£YPowerLawnone?íEÚrÛGm?¹(ÞÈ,<?µÑ,i%Ĝ?¹(ÞÈ,<?âUGŒUÜ?ÐBô¾¥º?ÛUqÒçTI?ÐBô¾¥º?ëќìEŸ-?§_"6É­Ã?À¹ŒNéƒM?§_"6É­Ã?áj¾ÿüòQ?°.Ø ¤ —?Ý*'^?°.Ø ¤ —?è7èª<³?ÊA¥èɔ?Ï \õW
6?ÊA¥èɔ?Åö™*o%Ž?̶¥¢çK?ê'Yµd6?̶¥¢çK?å%t?¹rîÃ0?Õµ÷ùñÉ?¹rîÃ0?­,!Å?šaÂ,¡î?î-?½žö??šaÂ,¡îMIXED3FGL J2030.5-1439@>Mã†Lµ»À<nš€If{À:¨ÂD³Ž7À;ÕäbÈ¿×Ûâ"Då@
h³'Š2ž?ý×>Ý
ˆ¿´SÅ)Åj¿Íºòºr,B¿àÒ­›rüf¿ØZg!ËËUNASNone@²èoß;dZPowerLawnone?ïýŠfYÑ?1¿6Aäùó?3¯uúu›_?1¿6Aäùó?ï—kÿ$d?¦L]¹Š?Š%AM»?¦L]¹Š?ïºrè%?}_žïÄq}?cO&wÇ?}_žïÄq}?ïüÏžÞ¨?&Îé#U?9‡yim6?&Îé#U?ïúKl~È!?GFW]£	?FÒMCè Ö?GFW]£	?îx6Žm§´?µç6-Úù?¨|—Iº?µç6-Úù?ïq–!XÙû?‹EܜèGk?'Í;ÔäÀ¬?‹EܜèGk?ïànÖ³'¤?eà?o')qŠ$:?eàAGN3FGL J2033.3+4348c@TœŒ" Ú@Ü@Þ¡À9Ý©"â À:aþ£®$?çbŽÀwª@
c¤&œ@ð»`å5?ï÷Ž›Ðù¿ë¬Î
 ©¿áÀø´îc¿ãmϟ™UNASNone@®'\(öPowerLawnone8?ïš·kö?–ˆ¸îZ?‰{2."?–ˆ¸îZ?ï嘱ÎU?©†‰Õtê?#LîíŸZ?©†‰Õtê?땶àý0m?­™1Êsµ?Á©$|>M?­™1Êsµ?îâåc­µ—?…ÔLq¦?¡Ñ©Âñ›?…ÔLq¦?íÿ9"kúq?³Qî0àø?°3cVQö?³Qî0àø?êƒâaš¶?ǕDäû0§?Åó¼vy•)?ǕDäû0§?éØçÁVZ?±Äðy¬·?Ȝ`ú§â™?±Äðy¬·?êÙè'q0?®ø-"0ü?Ę]ö;—A?®ø-"0üAGN3FGL J2034.6-4202@vq9C¬ÅÀB0øµˆãiÀ:~L69xÀ;©Ù¿#–Þ?æ!;xjä"@
éåµüÑ¢?ÿ+žÔA
?íåÐ6c¿B¿ç&çEsý?¦®o§sE¿é"ªß½sUNASNone@¦±ýÙb·PowerLawnone?ïûŽ»34?Eb_ûUç"?AÅý	¸?Eb_ûUç"?ïj07!̦? ªPºÇUƒ?'¹ù~9C? ªPºÇUƒ?ïC؜ä¨?"y¿ß³l?œ—"å"3?"y¿ß³l?î×*í¥›—?Œ¯AÑ¥‡`?¢Q(9û'?Œ¯AÑ¥‡`?ïôjŠe?bkí`z2?W+Óé,Ç?bkí`z2?ìlátq
?Â=%S»WÉ?¼˜ô\w"ú?Â=%S»WÉ?îIeó‹
Ì?¡±T(@?«i Ã߇G?¡±T(@?죉'¹ó?±q‰ðC‡?ºç3³ê0i?±q‰ðC‡AGN3FGL J2035.6+3146@R5ËÿGs\À(IёXÀ9‡â3f^ÚÀ;Šyk%é?êTÕ£@…lP‹2Ï@fs€€C¿ë&FÌ'5¿ç¿¯æÀœp¿Ö50•ì]X¿æÓq†wuOUNASNone@"Å©"àßPowerLawnone?ïüñáÀ`??ÈÁ¦åü‹?8pðÿ®¼??ÈÁ¦åü‹?±¥Ú?š¢š½¥?‹–Çùx?š¢š½¥?m¬¼ó?…}=…³?ˆSä'a'<?…}=…³?ïÚÈïƒÂ?X1W‰ÔS?rò§Ú†À?X1W‰ÔS?ï݉ªì±?zH±QkÖ?q~;Œ'¹?zH±QkÖ?í|ö¯/"(?¼î' Vë'?´J…§w½?¼î' Vë'?îXn¯=ÎJ?¢åÛH‡û"?ªyÿY?¢åÛH‡û"?ï4*)\?Ž1¯Æã?™z¼"q?Ž1¯ÆãAGN3FGL J2035.8+4902@U­'#'@#M~8DÀ9Î.\3Ý}À;¨—š¼¿ê¢ä4â$@T(1ÍWŒ@Ãf?úìƿ䍙/*SÕ¿Î4Ÿ䦑¿æ¤
™¬Ë¿àˆàéiUNASNone@±ØáÊÀƒPowerLawnone?ïú­•Ïà~?MÊ-o«²Á?EI¨«"}?MÊ-o«²Á?ル:E˜ˆ?†PUq»H?€Y±}9ð?†PUq»H?ï†ûñ—KO?‡/«Üj¹,?ŽA"Mô+?‡/«Üj¹,?ïþÁѶ8?±¶ë?#îÖc!h?±¶ë?ïÞ';Ñ_?r)¶ŸqDp?pù¾Î)"´?r)¶ŸqDp?îÂ_±Œ.?³†*£ðõ?£Úð_?³†*£ðõ?î¡K]\¸¤?žl¶~Û?¥ëJ-¤½?žl¶~Û?ïê\eí«Ñ?aa.˜Â¢³?e£™éß?aa.˜Â¢³AGN3FGL J2036.8+4234c@ThÕ¥¹c?ïèV`^åiÀ8§1"ÉÿÀ:3\m¿ <?õ"åm,©+@
êÇ+£ù@"€U$ö¿Åˆk><{±¿é={Êaô£¿æ'˦þ'¿ç
Yûsÿ+UNASNone@©±©ûçmPowerLawnone9?Ԙÿ-¥³6?Ð<8[w[<?峀i-&e?Ð<8[w[<?Ýõ‹$`$?ÐZ"õ',­?á:mþÏî?ÐZ"õ',­?ãQT£gÆ?¶Ýȸ¢¸?Ù]V¹0s÷?¶Ýȸ¢¸?å4€—%\?¬ÍƒTSl?՗ÜþѵG?¬ÍƒTSl?¥þ»T[?²;–\Œîœ?î¯@B,J?²;–\Œîœ?»¬n.0ë?Á՟ŒÖEO?ìŠ2:9ã?Á՟ŒÖEO?ß6Pù0œÅ?¹í 6M¼C?àd׃g±ž?¹í 6M¼C?ÌY£j'æú?²	"³˜Ìª?èé—%vB?²	"³˜ÌªMIXED3FGL J2037.4+4132c@T7™E¶Ãv?ÒÙUÜ«g!À8˜-¹éÀ:2ÿâ£Î§?ê	ÑÇÞQ@
®¸–^ü@lÁÅm2?Âí'f²wÈ¿èôöЖ¿äM{‡F ¿äoñÆg"UNASNone@°ME¡ÊÁPowerLawnone ?ã¥ì?ÒÝ{Øàί?Ù÷öµî'Õ?ÒÝ{Øàί?î›ðN1;a?±?ßð¿;?¦@ûìIë?±?ßð¿;?åƒìÛNß{?·/¸çì?Ôø&IbA
?·/¸çì?íå<Ó£‰:?ŽMN`Œçí?°Öd›",?ŽMN`Œçí?Õ7 Rñ??Ϥ²9×à?åd}/ևa?Ϥ²9×à?æF^JÛgè?ÍGô`dš?ÓsCjI01?ÍGô`dš?âðÜ4Z?¸ž‡z¾ø?ÚüG—Kê?¸ž‡z¾ø?å2€½¢î?³†œJœ?՚þ"»ø$?³†œJœMIXED3FGL J2038.8-3613@"o›™NÀB5™€o&)À9§ßV<L·À;ªÍv?ø>¿¼'ZqKØØ@
@6Tû¯ä@•P?ÞgT¿ä'@Ö½o¿ã	F? ô¿éÛIq&ù¿ä×›¡KUNASNone@…;å`A‰7PowerLawnone?ïê§ ?æu?y.9k¡?eXßÚ6'ò?y.9k¡?ïëQŽ#U?'aP‡>é™?~*WIlui?'aP‡>é™?ïCLLØ\?ºœjüš'?—–|=D,u?ºœjüš'?ïÇ[ÁR?gIï(<˜?|Rp×X??gIï(<˜?îè$ÕU/?¬·%q~?¡}²¨X?¬·%q~?îŒtETÑq?²Uü²~Ô?§8»­Fê?²Uü²~Ô?ìØ/Ÿˆy"?¬ÑJdAþ?¹>ƒN?Þ?¬ÑJdAþ?ì9 p@?®œ¸Gë¸?¾7.ü}û•?®œ¸Gë¸AGN3FGL J2039.7+1237@L¿/˜sÿ¬À12vd
k"À:`ýŸÓo~À;®QC¿rq¿õÃ{胷…@ò…¶Æ'@Ç«_ê¡I¿æ÷쌡¿í"ccÉöP?ÔÝ!yJf¿í˜[¿Õ~³UNASNone@¦öì¥zxlPowerLawnone?ïäM$©‹2?lo#XӋ?k²Û/ù.`?lo#XӋ?ïÝ.fM?œ·Íþ÷?ˆˆ¿E"xŒ?œ·Íþ÷?턃ã¥?¡"dR8QÃ?³ÛçØ°Õ?¡"dR8QÃ?ïÿ±¹Ô€(?öÿ(†Ç¢?'wV?öÿ(†Ç¢?ïßÞRq?tʋlÃÂI?pÿCy÷È?tʋlÃÂI?íþ49æ?ºÎ¥C?°Þ]W™Ñ?ºÎ¥C?í|å?®=?¥ò$Žyf?´ÖrÀ?¥ò$Žyf?ïý–Gß?A1†œ¸«¿?3OFoڀ?A1†œ¸«¿AGN3FGL J2042.3-5416@u{êüÎXÀBÞj㣨çÀ: jOÿò"À;¼àm"¿å±ÿ~GP@
¤ќj@lŠ I6¿â‰	Ú
¿ç"¡ì#¿éky˞¿ïû:%•»¿UNASNone@†r쿱[WPowerLawnone?ïíP¤C|é?g(‹Zý˜?b¯[Âw^?g(‹Zý˜?ï͍g¹Ï?Øt	Œýœ?y9LRð?Øt	Œýœ?îûrìJ…N?ŽaìüdŒi? HÑ<3'?ŽaìüdŒi?ïõ¦@éL?DZäØk±®?UʳZqxÜ?DZäØk±®?ïóÁ2º½V?`ux-]c?X}šS‹"ß?`ux-]c?îþ'kåèc?±˜cÛ{ú? ‰D5.Î?±˜cÛ{ú?î…Ë#²ë-?œæcãŽä?§£MÂ=˜5?œæcãŽä?ïìrm"?'…ÛqŒQ‹?Ÿ"qÁy·›?'…ÛqŒQ‹AGN3FGL J2043.6+0001@GNE^®âÀ8¸*º¾­OÀ:•sÔãòƒÀ;µ¤(hÔÖ?ëiG¡K·@
Ô爏Ü?ûÚ>ÐJ[?ÔSÙI:&?˜,Ɵ›˜ ?Èïx?Ï¿ãòJéÄe†UNASNone@¶‰#S÷ÎÙPowerLawnone?ïòÞà±ÂA?aÈêcçS1?ZB>9†¿c?aÈêcçS1?ï:ã_z'Ó?¤õc‡Îeà?˜£"š="?¤õc‡Îeà?ïšo9ô˜n?à¤ÀË)?‰d1‰¹"?à¤ÀË)?ïaLÑY?~Óރ•`¤?"ßܖeÔè?~Óރ•`¤?ïÚº
ÓB³?z.ËB£=?r¢ú¯Ë†?z.ËB£=?ì#ÊËsd?ÃlC¦"ï?¾á©¤dßå?ÃlC¦"ï?îÊpc_ ?›é"úŒ_?£XþÊ¥ôÿ?›é"úŒ_?îäc^õ÷?›e`€>õ?¡¹ÊÓé"?›e`€>õAGN3FGL J2043.8-4801@uúw1ÅÀC!²_c<æÀ9¢îRX'hÀ;³ Œgï?ññ[!ŽÆ@|¶M"m8@ó‰à%¢¿åŸGŒí ¿Êx=3<B{¿æVH«•p¿ïÿÜ^o³UNASNone@'OÛÚQÎPowerLawnone?×C~¯Þ?ÐJ<¬¦?äxö^@¨?ÐJ<¬¦?ÑIlw™áà?Ñýx³'a?ç[IÄ3?Ñýx³'a?å/Ç[§NA?±²'¿7 ?Õ qH±c?±²'¿7 ?Ów]–`³?¬
mP
e|?æDQ4ϧ?¬
mP
e|?Êl3§CȤ?ËƗËۃ?édó/
×?ËƗËۃ?¹;{6o7L?Ųþ‡&qÑ?ìؐ˜ûW?Ųþ‡&qÑ?Ô¬¶ºÅ@ð?¶ç'ʛú?婤¢_ˆ?¶ç'ʛú?áŽ°~O?‰ö§­&Àé?ïóŠH:N?‰ö§­&ÀéMIXED3FGL J2044.0+1035@L)©~+VÀ32;yRÒ5À:r‰ŠWÝÀ;– f<tû?èݗÿÕQš@Fýo,Æ@S§`Ÿþ¿Æ
 œO#¿å¶ˆSåÊ¿ÙKY¥bЅ¿ïÿûC¾×ÓUNASNone@•Âq²•êPowerLawnone?ïç-ÈT?ƒeÏ¿à?hÒ7Ìö?n?ƒeÏ¿à?î«IäòÕÂ?®SÄ0ó.?¥Ka±®ŠÙ?®SÄ0ó.?ìȇÍX&Ì?¤þ²k*N?¹»Á•>ɝ?¤þ²k*N?îƒP̘–Ý?†½̵…?§Êó7Ry5?†½̵…?ï¨9tëºN?›œ™,†5?…ñ¢ÈŠ?›œ™,†5?è].Vè?Êa=ÅæÝ"?΋G¾§è^?Êa=ÅæÝ"?ë~àƲ_?¬Ì÷–¯Ag?Â|å6ƒ¨?¬Ì÷–¯Ag?éæ2÷ ?³'µ¡#
?Èg4#•}Î?³'µ¡#
AGN3FGL J2045.6-6838@t`⡵ÇÎÀA¶Ü­¡À:kYnLÀ;¸à°¯_Ô?Äõ¿&,K@‰³*º=Ô@$¿²‡ý¿âú©/tóÙ¿ã'ú±À	£¿âê
ªþÆÅ¿ïÿóºÄ®éUNASNone@'#yÛ"ÐåPowerLawnone?﹪Pÿ…?˜‰Y®½°4?•k¼°'¼?˜‰Y®½°4?ïÆ<C
'?Ÿ;ñ¨?|áÞr_Ř?Ÿ;ñ¨?îFm7Äp?žµ¼§0¶?«™,'1	?žµ¼§0¶?ï½×å%'?c¨:.?§?€Š'µ[?c¨:.?§?ïɨ ü?Ž#·¼Ä?{s«£ü‹?Ž#·¼Ä?î´ûXa§ ?³3¡1ÝUƒ?¤°J{[û?³3¡1ÝUƒ?í/vÌKXÕ?¨']•´?¶"I¥9W?¨']•´?í" ¯*®? @úÔÄ~O?³fú‡ôjE? @úÔÄ~OAGN3FGL J2046.7-4259@vaŸ!-w2ÀCV4XÍÀ:mGÞ»ãÀ;Íw=N?(?Ö>éÜ°£@
ã͍@T kDò¿ç›s³¿×|žjÓwP¿×ƒ¤a–v¿è_¤]ö]óUNASNone@¢ÂÏùrGEPowerLawnone?ïþS¡#?+>Ñ?*ÅïNd?+>Ñ?ïµÊ,g?•ëÝ2už?'¾
yµ­‡?•ëÝ2už?ïÒYZ—[?u¬^oXr?vÓRØÖú…?u¬^oXr?ï–Æm.£ú?m§'¼ýa?ŠNd´W'?m§'¼ýa?ïú˜'æ?P´F¹
ï»?G'ŸpS?P´F¹
ï»?í½ÜânŸ›?¹Çâd0"ª?²ífê(?¹Çâd0"ª?ï¦ðè
?‡"àô¸Sb?†CƨËw?‡"àô¸Sb?ìÞ$,Òhe?¥™pøè=ÿ?¹ޘÕÝ?¥™pøè=ÿAGN3FGL J2047.9-3119@)©IÆónøÀB°>ž¡À9Äz•ÈSÁÀ;«zl­¨D?ê…ªÉÜq@RÊ/cšÚ@*zàEûb¿êþLÂY	¿á[_Ñïó¿ã"Åãà Ð¿Ü˛Lª±"UNASNone@"éßö"FPowerLawnone?ïöºqy•?YŽŽÖâm?R‹ù ýÕp?YŽŽÖâm?ïm…jžÀ†?ŸÉþ¸Ã…š?'OR³'1?ŸÉþ¸Ã…š?ïh¤KEÅÿ?$§»V"ò?'ëv•r?$§»V"ò?îÆ0(ÅN²?†!nõ&Û?£œýubâá?†!nõ&Û?ïޗ
Ú4Ð?xšôm¦¸?p´z|èà?xšôm¦¸?êºbÓñ?È	Ý'қ³?Åw°;ò?È	Ý'қ³?í†p±\ȝ?¤éºd–µ?³Ìzvщ?¤éºd–µ?èsõ´çA²?´æPZ‰¯?Î0),bù8?´æPZ‰¯AGN3FGL J2053.1+6027@XV'Ìö¾8@$"òsPÀ9KŽÀøƒ4À;S"9-H8¿"ø¨ÀŒ°@&§}‡ë@W§Å¬¿ä¦!'ÕbÑ¿çÃOÍ¥¿¿è_¯ðjƒ#¿ä͚ŽGgUNASNone@|ÖÓ›fùPowerLawnone	?ïüõ*}ÆÄ?9
ºmcóð?8V®Ã?9
ºmcóð?ïÂgæeœ‰?ŠOÿÉX¶ì?~ÌÒÓ`?ŠOÿÉX¶ì?ï¬x,ü&E?~"	GR€%?"áôÇÕ¦—?~"	GR€%?ïØG'~'¬?ZA×è£ß?sÜ>¥oJB?ZA×è£ß?ïä'M恙?qa	ä§?kرþ‡›?qa	ä§?îZ`Cëò?µ¾šøç?ªYûÃâÕ?µ¾šøç?î·ç^.Å¡?œfè\ïF?¤Š7¾ê?œfè\ïF?íÀýŠ(l? »Æ$}f?±ø­žîŸ? »Æ$}fAGN3FGL J2053.4-4052?íUÅߝ´ÜÀCä¦">jÀ:Yt^v­ÜÀ;Òù=¼¿Ä©ñÍڋI@4؃9Zë@TF__áè¿ä—I$_þ¿ß/.©9¸¿â†g1ßÃl¿ïÿÀtFEVUNASNone@'Eê³g ùPowerLawnone?ïàsñid?|oKÚÏdò?orŒ•[©?|oKÚÏdò?ïÅÜ˝wË?˜:å)˜?}š<òƧ?˜:å)˜?í1aƒÊò¤?¢M@¹NWá?¶tóãÎ,Z?¢M@¹NWá?ïÏB¹?bPÁ`ur0?xz€[ƒi?bPÁ`ur0?ïØ.»æ[Ð?L?©M=¹?sè¢	b{á?L?©M=¹?î×.‹6]?±àÙEÂ\$?¢Mvá?±àÙEÂ\$?ëkûÔLH?±5Áj"
?ÂP®Îß÷?±5Áj"
?íÝ×࿞?¡"À	•s?±GÐ?¡"À	•sAGN3FGL J2053.9+2922@RWâCV—À#»
QøXÀ9ÖV>Ðö'À;V±AV¥?óÙ£A«q@ŸÝq§?ø²€@LÜ¿á훨´â?ïþpßÍ@Ì?ÊGɉ1¨«¿Ùµíkí}¶UNASNone@—Rn—PPowerLawnone?ïN'}"vX?¡*P0{C?–/°JIË?¡*P0{C?íËo()	?¹¸ûaYë?±¤†ÀJžº?¹¸ûaYë?î"îò32?Ÿìz>å?­ÑÜϬÚ?Ÿìz>å?îYEhCr?"aŒÎ4Iì?ªk®êW¯ç?"aŒÎ4Iì?îp#âï_/?­…fmû?¨ýÁÏR??­…fmû?èÑې›)?ÍÿånëVa?Íȸ'½"Z?ÍÿånëVa?ìö­˜¡nr?¦ûýlöÐ?¸J";bó?¦ûýlöÐ?íªéq·í?©¯¢³]_ä?²¨´r@—Ó?©¯¢³]_äAGN3FGL J2054.3+6907@Zð¿\£@.Ÿ¾˜V£{À9ìÆ%鞕À;¤¡pþoÝ?Þ>ü³"	s@¶Š{C˜0@ªx z´Q¿ì8¦O¾ò¿—rÍËüøw¿í£­n¸š¿æ@²ôDÇUNASNone@‰nËûµPowerLawnone?ïì»æ(F#?r"Î)BíY?cD•Á]"?r"Î)BíY?ï#¼LçÃ?¤OB²|öh?›ˆv~"?¤OB²|öh?ï"ÆjÅ?'æÂ3š÷?Ÿ[§;ZÙq?'æÂ3š÷?íXÀVOu'?—¦Ý£)}a?µ9ýN`:q?—¦Ý£)}a?íÿpV:…?³ï¡sm?°l~*Ó?³ï¡sm?æ'Î\L®?Îï˜Í8O?ÒúcGfà¤?Îï˜Í8O?ì#mÎo?«†ç=ÐëÌ?¾ä—я̉?«†ç=ÐëÌ?׍xm=ßÎ?¾9'"Я?ä9CÉa?¾9'"ЯMIXED3FGL J2054.8-4908@uâ'RT`ªÀD‹«`kÀ:?ø³o.À;¹wD;Ï¿ùAž‹EîÍ@P!ˆ¬6@ސ>&¿ê%£"˜ÅM¿çLèdi_¿ÎB×Ë®iµ¿ê"gƒqäõUNASNone@•(Þ5?|îPowerLawnone?ïýx‰Ëé?5š0´ä™q?7L;!—'i?5š0´ä™q?ïјëì;?½°M…ÜÞ?w3Šðâ‰?½°M…ÜÞ?¸\
®?ƒ'-ãà´?ŒÝÑóKhi?ƒ'-ãà´?ïÿà#îó>é)­' ö>ïíÚÎ)§>é)­' ö?ïý¹¯—:w?8ú\ÅÉ«Ò?22'/ÿ?8ú\ÅÉ«Ò?ï+%Ôa&ó?°û1Ç?š›EsÛ!­?°û1Ç?ï)©¯f_…?"fª¨¦?šÊÊëÝO?"fª¨¦?ïþSŒ2í'?)»'¢G
c?*Ç=mISÜ?)»'¢G
cAGN3FGL J2055.6+1609@OlUÚ'(cÀ2KÈâ\
À:+òËdÀ;¢Y£àDy¿ó7‡mò÷¯@
‹fNJBº@ö_ÊëÌ¿ç
y]0¿éØyti¿â=Œ˜TJ/¿à\¢ÿã"SUNASNone@‹E‹]ÌcñPowerLawnone?ïÿlԏì?½8¢Õ×?e'
aEŸ?½8¢Õ×?ï­=.ÿí?•Coîç?"°´o10è?•Coîç?ïÙTÒëò?id½ÍZ'?sU–¤Ž¬?id½ÍZ'?ïÿ:ý›»>ýÒ!¹'?±Qa)Ã>ýÒ!¹'?ïþ‹1ˆƒ?.¾_å3L?'LåV#\Š?.¾_å3L?î\¾ˆw™{?·h,PÑ?ª4uÌX?·h,PÑ?ïzïå"%'?Œöðÿ?¢bš…Ñ?Œöðÿ?ïøÝ^6äe?HÔf‡á;?LŠˆ…Ý›?HÔf‡á;AGN3FGL J2056.3-5925@u6;%oüÀCm'Èâ]À:*¤L{ÖÀ;áà'ód?ò'ål€Ü´@óùˆl '@ir"¢?¶rj5òµ¿ãDè›pšƒ¿æ¦üP¿ïÿÒ`_'5UNASNone@zŁoPowerLawnone?âÓº4ÍDÊ?Îúsà2Á?ÚX‹–evk?Îúsà2Á?Ø(&Ý÷]?ÐÄR§?ãëì'}Q?ÐÄR§?沧 Ô‡'?²š¾¶0?Қ°¾VðÛ?²š¾¶0?ÜwVZ¢o?­Ú¾5ãÅ?áÄTÒ®ýÉ?­Ú¾5ãÅ?×|¿]lÔ?Îöw*®Õ@?äA QwI–?Îöw*®Õ@?ÀÑ´×ÒS8?Ç°[½k?ë˒Êk2?Ç°[½k?Øvãrfá?ºå«'¤éÀ?ãýDŽF̐?ºå«'¤éÀ?°@õD |ˆ?—öE–²ë?í÷áW78??—öE–²ëMIXED3FGL J2058.0+4347@U@dÜY2¿ó¬§
£3À8$óĈ[À:È	€²B?Ú¶óƒè#ã@݊µ%;@\¥ÀC|'¿ç;	XØݿ뎵jZ'Ç¿ïþh#¼?ï½IÓnãŸUNASNone@n&mŒ?PowerLawnone?ïì3M
!?mSl]$4?c̲½ÛVù?mSl]$4?ï¦y\¾-?•x+…ò?†a¸öŽä ?•x+…ò?ì¨ì¤È:±?§*ƒ++?º¸šÙ¾*{?§*ƒ++?ïûË·ñ?ë?Dý‹Ún{?@ÑbeÁ~?Dý‹Ún{?íS@ƒ?»zKܳ†?µeÿj,9\?»zKܳ†?íÈá`Åà?»Q'(¹²"?±¸ó±žþ?»Q'(¹²"?çl$K8ãv?·&ؖ`}d?Ñ'·iŽ9?·&ؖ`}d?ïgXA"%ë?¢Ž€@?%Ô?"÷Ö2HŸ?¢Ž€@?%ÔAGN3FGL J2058.3+3729@T
™E¶ÃÀ†wc
ìRÀ90/JpfšÀ;;Ð<ÃÕ­?åðÑgñq@
ÝâÃJb@šåÀŽ¥ö¿íÀ°º¦L¿æz[>¦?+¿ÞèúÇÔ6ñ¿â]Àc÷	UNASNone@rBÄGÃ
PowerLawnone	?ïú¢d™]?K-FÙR?T?G½u½!Ñ]?K-FÙR?T?îƒ1ÐÝ}Ÿ?´ÓŒB–&?§Ìâ?´ÓŒB–&?ï]ϐÃÔx?NAÞEí?"F
ì¬Úø?NAÞEí?î~•@]W
?ˆg8ÚxBB?¨«ü¾D-?ˆg8ÚxBB?ïÔ¬^å‹?€Ø'½—¦?u©Ð‰÷w?€Ø'½—¦?å? ¢j1?ÐITÝZ—?Ձ¾»*ýž?ÐITÝZ—?íÆĜ@¿?£?5O6+Þ?±ÉÛ³À?£?5O6+Þ?ço ¿ñ¥¨?µâ"ý?Ñ!¾€´°?µâ"ýAGN3FGL J2059.9+2029@PÇQ'©"À0}°5½Q/À9öÚ˓À;…OºRvÅ¿ú&"î9.@hÛkv¹@œàŸ©¿ã²ÍN@ą¿ìr‹FÖº¿ßëtbS¿áÈAŽDUNASNone@†Û¸B0üøPowerLawnone?ïÿBìAdØ?ˆð£ê—8?¢|÷ºÝÃ?ˆð£ê—8?ïº'ëν	?' +Bí?v	9®?' +Bí?ïÐYÌFŒy?oîgþ|?wÓÑ»¯?oîgþ|?ïÿÓÂ+Öj>ðÒH‰Þa(>öìb!˜s>ðÒH‰Þa(?ïþ:g¯è?4ºŽcé¼Ø?/ìX2[<?4ºŽcé¼Ø?î›8?·{?´þA#‹ËP?¦L|d6ï?´þA#‹ËP?ïYñ
§f?¾¹ÊͪT?"ÁÞLËŒ?¾¹ÊͪT?ïü/»Úa5?=íxêöÇS?>'gö§x?=íxêöÇSAGN3FGL J2100.6-7844@s£Á½¥À@W±B,Ë:À:vë»ÛÀ;¨¥º9LR¿Õè6W!qa@éÙM
Ð@Ú]ÿ—¸¿ëF|ˆ‰m¿èⰠě¦¿ãš&É\C½¿Ý"¤[OÃUNASNone@~vö"Fs'PowerLawnone?ïÿ›¡å 3?uï7›?	•­ÄÍ?uï7›?ïÎüPYDü?²š{Ô¨2?x×½`'?²š{Ô¨2?ïåÖÔÁ'?[¡ ¤|Øã?j)+C	õä?[¡ ¤|Øã?ïýJ
»ò? Ö²åúJI?5¯©Ï? Ö²åúJI?ïÿ·(ScÞ?Qß}#é?5ë^g?Qß}#é?ï/­Ä7Á§?°­Éì›?š
GžÑ?°­Éì›?ïÓçÖß~?uYy›³?vtöS±;?uYy›³?ïàýmtU?aU)ZÊÚb?o'®Ò;¦?aU)ZÊÚbAGN3FGL J2102.8+4704@V:§›ºÜ?Òë|eVFÀ9]»JÄIqÀ:üÅCk›?é/ÇÛ÷7/@ŠaÎQ1@'ÿ\—¿åև¶¼©¿ÈšUÅô¿ãQ˜ahÙ;¿â«RyÓYUNASNone@ªÚQÎPowerLawnone?ï÷d°2?NF2-•‹?PÅ8KÓj"?NF2-•‹?ï'±Ôßý?¥jM]£@¯?œ-ÉÈӜ^?¥jM]£@¯?ïã§ý?‡~•úV1‹?Œ‡žòÙ?‡~•úV1‹?lÍß?'ánV_1?¦ÔUÆ?'ánV_1?ﶋàüã?'ŠÙ¤¬á5?'zœúWL?'ŠÙ¤¬á5?è¤~—0N?Éú;‡Œô?Ín£û>È?Éú;‡Œô?î"zâ°u?¢+å{¹A§?­ØQÓ@á?¢+å{¹A§?çÉb]~q†?¯\åa­¿Í?Ðm;Eô?¯\åa­¿ÍAGN3FGL J2104.7+2113@Q <K	êÀ0çr>á½À:\%ĵ§À;¤¬°Í"À¾|¥-Ì@Hÿœ'Ø@iÀÎO?ã߻зNG¿Õïãð!]¿èñ¾
‰"4¿­t4Cú6ÛUNASNone@®Ö$Âø7µPowerLawnone?ïùôL?NC@íÈÝ?H/¾ñÀÒH?NC@íÈÝ?ï½Í6îÃ[?'½uÑDT?€Œ²Ay&?'½uÑDT?ïnîÚ¶ë?"»Ô"%ó@?'"$®eL™?"»Ô"%ó@?ïÿÿc;ÓZ>˜ëÉ«
-\>"Ÿà˜—cp>˜ëÉ«
-\?ïÏw‡(±?~7ï^ê‡?x~Ä îÇz?~7ï^ê‡?
¥žÏ?³dÐèy÷I?¤7ß$Ê,?³dÐèy÷I?íÓg§jMã?¦~¡¸?±dÂÆÓRg?¦~¡¸?ïÿâ´`Î>ûîӜǎÜ>íïr¤

•>ûîӜǎÜAGN3FGL J2107.1+2248@Q…£Â‡èÀ0V2.oÀ9ýE= óÀ;‡ÙRMI¿æå®Zk@
"÷P®ï@Ïã ¡5D¿æ–
ìZdX¿ç ^F~¶â¿è™•Rë'é¿×}‡TUNASNone@‹‹ydoPowerLawnone?ïý´`Å<¶?9ãpÊ1‹?2\ûö®?9ãpÊ1‹?ﶈ²cŠ?•aŽÕ	K?']Óx3M?•aŽÕ	K?﮿ñrª?wçâ•G¦?"Pš‰™Ÿ?wçâ•G¦?ïþO>Š1û?wW9c ?+Эø}?wW9c ?ïï?î$ß?eNº,?`ÀøÚ؍?eNº,?îš,J¥"x?´Ú™Ü¦ß?¦];R8?´Ú™Ü¦ß?î¡d4¯©?ÿ­6éÒë?¥é¼¼qPs?ÿ­6éÒë?ïÛ\–ª?n,ìZ!WÀ?rQ´¿™Z?n,ìZ!WÀAGN3FGL J2108.1+5202@WTów[@ÒÜʵ›À8n†º™ÄbÀ:³×û뿼« ÜrËé@/îWŒ@v7]d¿ßëŸTR¿êöò·åV~¿ä¦ª™q*»¿îݓ»Ö}UNASNone@'‡ [ÀPowerLawnone?çFºfîk?Î@Eт?Ñr‹2x£*?Î@Eт?ï©b¾!t€?"˜Ah?…§Pt3Cÿ?"˜Ah?èyoÛ/;,?³]–èà	Þ?Î@"CP?³]–èà	Þ?ïÉo˜\©?eíß=ڂ?{H3Ô¥?eíß=ڂ?毭³"&?Éwß
?Ò ¤˜Ù³Ä?Éwß
?}¬?·òhìNþ?¯ÅY
|>?·òhìNþ?æbª³â	?·áÆ­C²—?Óÿ:ª˜;î?·áÆ­C²—?íœT³FÐ? ¸—¸MKÔ?³Zf¥fÜ? ¸—¸MKÔAGN3FGL J2109.4+1437@OØ$>úèÀ5áŸâÚUÀ9NØ9¦ëÀ;"wÏDvÀ`Z"°ÔI@|p¿…¼m@ÜŸ‰Ê¿å>KïA¿ì²HČXá¿â"ÿ½ÿ™B¿æUÂ`ˆ7UNASNone@{Û䎊qÞPowerLawnone?ïÿæÏJx>溞µÖ[>é0Ü%‹ok>溞µÖ[?ïÂÓLË5?ŒÜÃh^³÷?~–|Ô¤?ŒÜÃh^³÷?ïë{OÆU©?f|1 ­ÎF?d"°^Æ´?f|1 ­ÎF?ïÿÿ䞝>s;2  >k}bÎXÍ>s;2  ?ïÿà.˜2«>ïˎ6Vø'>ïч…ℱ>ïˎ6Vø'?îÑ'C<s?³avëÙR?¢îî_íÇ?³avëÙR?ïØ·pçk+?u¡1n+D?s¤G"‰zk?u¡1n+D?ïÿý"üâû>¼Sû";>³Y=U;põ>¼Sû";AGN3FGL J2110.0+0442@Kx"ÄGÃ
À;Ö2.oÀ:;÷ƒY¼4À;³{ë2éa¿á&æxFä@³ªÎJP[@cŸâˆ÷¿à¸94
§¿åEø(<¬¿Ù
´ë?寿ګ贒vîUNASNone@£Êéã½PowerLawnone?ïÿ'Ñ?âuXhÓ¹?y~'àù1?âuXhÓ¹?ﯳ¨R^?•-"'í£Ÿ?"?SÚd|?•-"'í£Ÿ?ïÞo–)¼V?w_Æ♒	?pÈ4êqé?w_Æ♒	?ïÿ),ìV?0µP},H?Úq¶w?0µP},H?ïÿu¥ì/?#
YÌç?K\‰p?#
YÌç?î}É16Ù±?·—Dµ?¨#léþ¯ö?·—Dµ?ï˜X#W÷?¬1
ùnÀ?‰é÷Zk?¬1
ùnÀ?ïù^]$ë"?B†-ºyR?J†ŒExþ?B†-ºyRAGN3FGL J2110.4+5946@X-Œ*EN@Þ͍¼ì…À9W/ ×{|À;5(ö™Nñ?ÏM٘žX+@'Ë+·é¼@EKYl-¿çõ[s"x¿ïē_e7µ?ëçÖ4÷Ñ¿ìÊÒ @3ÄUNASNone@ŠF¬¥zxlPowerLawnone?ïхƒ.•Œ?wTæÔ»Nº?w=>rT!ë?wTæÔ»Nº?ï°u- ?Ê_-cŵ?ƒâ´» "?Ê_-cŵ?î#l°q;?žÄ\ý]Ä?¯½É8hˆG?žÄ\ý]Ä?ïÜBÁ¼µ?o':	Ç1?qÞþ;Nq'?o':	Ç1?Ànçâ?B>Õ-‹?ˆ"ÝfÏ¢?B>Õ-‹?înþ/ÆAB?´ÙûbÑ\?©,OÞ?´ÙûbÑ\?ìðÌrV?¨ê‹9.ŸÑ?¸yŸc&"Ñ?¨ê‹9.ŸÑ?ï á­À©9?Ÿ®ÖeÔz~?‡Ç"Õ±´?Ÿ®ÖeÔz~AGN3FGL J2115.2+1215@OM'#[NÛÀ8scä«æ£À:¯çÜôÀ;§Þ7X[â?×:m-n¼æ@6W'¸ÿ»@JN LO¿ã°Ì)Au¿é"Æ gƒ¿Ù¼%UÿÝJ{ñŠiUNASNone@¡hÆffffPowerLawnone?ïÿ]#$Oô?Ú¼h'Ÿ?[Ÿ¢»+0?Ú¼h'Ÿ?ïàO"?¢a¡'§á?‹ÇýÞ|G…?¢a¡'§á?ïçý‹D?j–FZ,ÉC?htô{–ê?j–FZ,ÉC?ïÛ|L¤‹?V°vƒS­?rAÙñMâ˜?V°vƒS­?ïþI=zx±?/¼<¿R]q?+l(Dªe¥?/¼<¿R]q?í©¹F¡?»`®ß""?²²5˕Ÿw?»`®ß""?ïËzCH?}!¶{­'?zzCë?}!¶{­'?ïïnjõJ?ŽÂøè©?Ÿb9€Ž¸?ŽÂøè©AGN3FGL J2116.2+4422@Uél <K
À
=›l±À9ŠáçDòÀ;J¼¼´Q?ê¶çnþTH@
œÚ–Ž¢@ô÷í¿î°±A𪿿ӺãÒ^¿ç(þ'jöï¿Ñrž<W8UNASNone@z£n.²PowerLawnone?ï"VÚµÌ3?¦t I#Ø?›µ$®mãŸ?¦t I#Ø?îÙ\`º;6?°Äš¨|$X?¢j9ó€e¢?°Äš¨|$X?îZ~Ú.=?žÜ¶ülŒ?®X™8?žÜ¶ülŒ?îôå9w'U?‡¶ÄýV ? ±¬gªó¯?‡¶ÄýV ?ꌘdeZM?Æ!àòÀôŸ?Å͞nj–Í?Æ!àòÀôŸ?æ麵.[Ä?Ïî2£n?Ò,Š•£Hx?Ïî2£n?é6£ù«
?²†Qcó×?Ë'ÝpSÊ?²†Qcó×?èê*ÛmEö?»¸i«$ ?ÌWT'Jè(?»¸i«$ AGN3FGL J2116.9+1343@P	:¼"peÀ7Ü¢G'ÝÀ:/–WZZÀ;£æÎ-¿ü½¡'	Ó@ä–'IE@ØÍ¿àVôï^OÊ¿ã²íáx-¿á}-eeé¿ê™Š]ÅUNASNone@–,-«ŸU›PowerLawnone?ïï¨æ#ò	?]
òa×Þ?`W÷Š×?]
òa×Þ?ﻬߥ<?Mj…ÉœÛ?È$v Ô?Mj…ÉœÛ?ï;±=ií?ŽõþØJ ?˜‰ØM·Øo?ŽõþØJ ?ïÿÊ,"a™>ö…m¸G>úê©s&1>ö…m¸G?ï´lÅ¿×
?…ÿÔÍ0è?'äΌò—?…ÿÔÍ0è?îÃo¼"ë?³J¦3´L?£É8›hV?³J¦3´L?íÄS×m?¥«Z‰~?·™Ý`Ö ?¥«Z‰~?ïú¨ž€ob?E¢œ?dÒ?E]†FÓÐ?E¢œ?dÒAGN3FGL J2118.3+5751@XcR?gôÜ@¥XÂ8õÀ9pËæÀ;d ;ë¿Ô³"î'̉@ÙM(§¾ö@Ýé_—e¿æf"suÿ¿èƒ¤ª™Ç¿ÞXœóg¿é)÷ŒáFÏUNASNone@l‹]ÌcñPowerLawnone?ïú,¿¯5–?Hè)²ƒˆ?GM©;)Ï?Hè)²ƒˆ?ï¿iø0?Iô̸X`?€9¥†kxL?Iô̸X`?ï¤÷³LÀo?†q<ý8.Ø?†Â3¯?†q<ý8.Ø?ï÷‰43õ?:O~
¿ám?PíÁÜPDÞ?:O~
¿ám?ïòšG&Û?bO­y4É/?ZËq¡6ªº?bO­y4É/?^\'ä?²ô44\u?¤"š6ѽ?²ô44\u?îÍÓá¥2?œ`\³ †?£."ÅUHØ?œ`\³ †?ï±!C­ºõ?uÀ²ìì<?ƒ·¯"ÿž°?uÀ²ìì<AGN3FGL J2120.4-1256@Cxéö©?ÀCmS?B5/À9Ô¢ç 5*À;µšTbX?äìwþÐfF@È'qßÁ@" ©ƒG¿âD4ҏµ¿ê*¯8¿æ"J®êu¿ïöEI5SUNASNone@ÔÇâ'APowerLawnone?ïøä
8Ö>?M*'I*a?LoËǧ^?M*'I*a?ïsõ8âÛ¾?™Á»"Ù?'XêƒÀ4?™Á»"Ù?_0×?OøPµ?‰Zh3ùŠN?OøPµ?î¼+ûí‡é?RïêÔÚ?¤=@>"Ìl?RïêÔÚ?ï÷«Üxwœ?VƒçuW?P¨Fݖgñ?VƒçuW?ìaAú] ?¿!=u×H?¼õ÷Ø-þ?¿!=u×H?ï\¨´-ˆh?½W¿?"jévßVþ?½W¿?ç׿MsÚ?­ùØd(Ë0?ÐPçeL?­ùØd(Ë0AGN3FGL J2121.5-8253@sXm›äÍuÀ?M>EþÀ9ð¹£$\×À;q©Ä[åÀåèô>×@
T"ÆK(r@¤S_ùdÛ¿æ!Á½"ã'¿è…sä˓‰¿àpÓþ"ù¿éÏÐøFUNASNone@‰³KƧïžPowerLawnone?ï¶ÝÜ-²?´ÑÈ¥+æ;?'Hˆð(y?´ÑÈ¥+æ;?ïÓãÊjFñ?ŒSWËõ?vÐ[ç£?ŒSWËõ?ï€6‡·«?‰°Å¢dƒ?ò^d€?‰°Å¢dƒ?ïÿþWß:
>³ÅŒ+èÃ>ª~ÄTXH>³ÅŒ+èÃ?ïø¡ˆ6«õ?T®@••:?MyßLX‰f?T®@••:?ïI–Íj	<?­•ýîDü?–Í&Tv¦…?­•ýîDü?îëߤ7NÃ?–šß€ð?¡B»¯,Ï?–šß€ð?ïÿ½‹*?RÆNa7Ð?¼fÇå?RÆNa7ÐAGN3FGL J2127.1-5615@u9EÁ?ÐÐÀEÎtŸM¡À:QéõÒ"À;ÇæÿëÀH•7µ#
@
ô6¯"'®@""¿æzšûÄ\¿é¥Ù	·¿Ò³:«ˆÀ•¿ïÿÁ£›G'UNASNone@Šd%®æ2PowerLawnone?ïûrñx§?E¾­ S?B4<‰r¤?E¾­ S?ïÖ;ÕªR?ˆ¾!Á?tþâ )–Ö?ˆ¾!Á?îÒ8×~Ý?'fwÁÎ.?¢Ür'[Ç-?'fwÁÎ.?ïÿþõ¶Gr>¬Y`!Û!> £YdC5>¬Y`!Û!?ïþ
NЦ?AXݪÏ•?/ï)þ­?AXݪÏ•?ïGnZö??®èS³?—4¾8,?®èS³?ÂõÕÒ?œð:äM4 ?¦6ÌWæ?œð:äM4 ?ïÿÝ¡Ân5>ú3éÛ¶§>ñ/ ã7
>ú3éÛ¶§AGN3FGL J2127.5-6001@tê"ã¼Ó[ÀE:â–êÀ:Ç©Á/	ÙÀ<
œKû¿çš¼s°ž:@2"YŽ'©?ÿ5ºŸM¸›¿ç<íyÉ"¿Ï+@Ç+´J¿æú~˜®¯x¿Ìÿ)UNASNone@®ð|ú¬ÙèPowerLawnone?ïú£LuÏe?R:uÇU]5?ErÎ[ã?R:uÇU]5?ïÏýO1Ҝ?½Îºà&¡?xX{mÏ?½Îºà&¡?ï'S!îšÛ?@㧇&?‹«7‹8?@㧇&?ïýÿ¼°—Y?"ܪž R`?0"_uÂ?"ܪž R`?ïõÓÒáŸÿ?XÂ'ìŸ?TXZ†÷'?XÂ'ìŸ?ï/lô8æ??°}ñËÅø?šausœ?°}ñËÅø?ï2ߐÁ%?´"ðã,‹?™¼
çÛW?´"ðã,‹?ïÆ+$	äI?zÇÚfì²Á?|ên
,#S?zÇÚfì²ÁAGN3FGL J2130.4-4237@vgxÔýó¶ÀGWzÃë|»À9ŒíÀb[?À;©Äe©?ìGœÌ vå@•¼ÚçB@}´"9¼¿ãçÀ¡lh¿è"ïjÓÕÍ¿èý("Oý¼¿ïÿ¨óz÷UNASNone@ð•a'PowerLawnone?ïæ[Ëû
?«ÿ?ükŒ?i¤4²'Ž?«ÿ?ükŒ?ïÃ+¯—n?•Ú–£Ò?~j(G†Ï*?•Ú–£Ò?ïBeùŒ¦ö?‡`û þEs?—³@̳SR?‡`û þEs?ïàÂ@4?T¢*çǾ?o=¿²Á¶?T¢*çǾ?ïÿhs?Ç5îw–?ñ£îéz?Ç5îw–?îêËrړ	?³çí#‰?¡SHÑzèq?³çí#‰?ïGNhv?"JÌoe?ŸW»Z[,?"JÌoe?ïv2
Xu?'wE%âßQ?'9¾¸n
R?'wE%âßQAGN3FGL J2131.1-6625@tjD›¥ãTÀD#")³úÀ9¦*Í3$À;Õ8¶*?òŽ1^FÝ4@©X†~߯@""_öŠ¶¿Ùî)òJhb¿ä¸pL¡ÌÌ¿éÔÑß8貿ïÿä•|¯UNASNone@†0& YŸPowerLawnone?鯮¿y/Ê?Ɵ|l.Ÿ?ÉAE@×?Ɵ|l.Ÿ?á5ª	ºz ?ÐEåNë ?ݔ«ì‹À?ÐEåNë ?ê®Ì<Òz?ªÞ³ð³?ÅDÏж?ªÞ³ð³?áèsœYè?¬
t?Ýè/ÇL/?¬
t?âx8&sB~?Ðh`«UGŸ?ۏ³{?Ðh`«UGŸ?É$&®s#?ÍC·Kö?é¶öTc7;?ÍC·Kö?۷ɳ›V?»ÌÞ?ä"?â$&2Tø?»ÌÞ?ä"?´ëJ9<À-?œì˜«'0?íb–¸"¯Ë?œì˜«'0MIXED3FGL J2131.5+2605@S"wškP±À2F£"¯WÀ:)ë°½¢À;ƒŽÝ}ôø¿Û™Œ;Ê@óÝq	Øq@(¹_\±Ý?ï×*æ!va¿çÎk·mv¿åé{ÜÅ=a¿¶¿µÑ_búUNASNone@›hۋ¬PowerLawnone?ïüÙfÛx¯?Cm—ñu@Û?94ɪ^~*?Cm—ñu@Û?ﷂ»å&"?•­1ךK?'PýÇ_0?•­1ךK?ïpW/¢ì?†ú8ieæ?'ü•"¢¨r?†ú8ieæ?ïþ5¬y	? ;ëïÅ?,¥;³Y‹? ;ëïÅ?ïçÕiÆ?wP´ùF}h?hì*ÀZê?wP´ùF}h?î¯ÜZΛ?´<ÜG^?¥:RB_O?´<ÜG^?í<κ/2À?°ˆv¼Iò½?¶Š.v?°ˆv¼Iò½?ïéx'»(?dÜ=ƒ?f‡ØôDØD?dÜ=ƒAGN3FGL J2133.6+2821@S£ëJwÀ1Q\éåâÀ:*`	UXÀ;›•]ʶr¿ñsp/g÷‹@¤ž™ˆ§¯@üɀ'±¿ã>úµ?	¿éòµht2¿ç–]Ê¿Ðô˜PæšUNASNone@…R?gôÜPowerLawnone?ïÿ—ô©? Ò:¡¢?Lþã
ª? Ò:¡¢?ïÂ	\Ë%?ê–UO9d?~ûQ†Ž±ª?ê–UO9d?ï»Q:bÚô?ywØ¯Ô ƒ?+±eéjõ?ywØ¯Ô ƒ?ïÿË°J¾ž>ð!j©Øž>ú'Ù"-¯>ð!j©Øž?ïûÿŽÚ½•?FVÈ—í³?@Äj(%"?FVÈ—í³?îÒÌ!eD?³ƒ÷ŠªW?¢Ó?@}`¸?³ƒ÷ŠªW?ïíýkrŒ?–Ö¬~áwù?B@[(´n?–Ö¬~áwù?ïûãd­˜n?>»uiôÐ&?@rlIûYÒ?>»uiôÐ&AGN3FGL J2134.5-2131@<ëÊû;u!ÀFŠœË}AtÀ9H£ÝÀ:À;¨jJ÷u¿ùñª—˜¸s@¥P+¼q`@`M¿Ø"9Ùô¿æaaÍX¿àâÍú–«ö¿Òéå,XèUNASNone@—TW$tSPowerLawnone?ïþ7<ú~®?,äâfÒWš?,Œ.¤­??,äâfÒWš?ïÑÏo"?^̸+µM?w~@í™î?^̸+µM?ïÉ£HU?‰?xóç…ð b?{.[ôü£v?xóç…ð b?ïÿðÎ^È7>Ùë~÷$NÑ>ÞbùPçÎ>Ùë~÷$NÑ?ïü/¤!L?B­À2hLG??æ€Ìþ±?B­À2hLG?ïT|ݲ^s?¡úö¶;»?•pdI´1©?¡úö¶;»?ï{ì,
þ?Œ^æóÈã?'zz6Ö@?Œ^æóÈã?ïþßÎ "Ï?#–ƒ¨·?"žäà[?#–ƒ¨·AGN3FGL J2135.6+5742@XÆÂÎFI@ҒwcåÀ9Zžˆã—À;ëóف¿®×¶Ý7®6@)nu©z@ÀôÌùî¿ça
ߤb¿îM:piI›¿Á.Õu½ÇK¿ÒA»X¨…UNASNone@…?žžšPowerLawnone?ïþÄÝ{Võ?,žÁøŽ–¹?#²*ÿAòô?,žÁøŽ–¹?ï·ÉFÊ(?'ñ8â«£‹?'
®Š³Ÿð?'ñ8â«£‹?ï¤'ÀÊq9?‡ks©`…(?†öÔBé³?‡ks©`…(?ïüåE‹?$@<×br?8×ÆLPc?$@<×br?ïüEž£LS?C.s5wË/?=ÓƒñÉð?C.s5wË/?î«­þë$?³z5hQ)?¥E.¡±¾?³z5hQ)?îڋÄòk?ž°Ç¥Éè<?¢WO°ÙI?ž°Ç¥Éè<?ïñâãåm-?S4çhY…­?\:7×°G/?S4çhY…­AGN3FGL J2138.2-4939@uÀE¡ÊÀƒÀGyÔbÃC·À:,õXQÀ;^ç$?âíÊ$"w@q†žj9@W*?nªÙ¿â¼V¹ä×t¿èª9G@Ô¿æ¼þ'"¿ïùÚmZ‡œUNASNone@"\´SŽóMPowerLawnone?ïá_ô\]Ï?yLñ¿-Nƒ?n Ö|hÑ?yLñ¿-Nƒ?ïŽZ(óò´?—ÉpQÓH?Œiu¸´?—ÉpQÓH?IZ?"ê>pÕµg?¥^Æ-",c?"ê>pÕµg?î>-ÈK?ˆÛ"· Ne?§ì¿·0E?ˆÛ"· Ne?ïÁ»\ÚC?ˆf0|Õ>?{¢g^e?ˆf0|Õ>?êb ®-F×?Çþ-Hž»?Æu}GJä¢?Çþ-Hž»?ìCMBÅ?«¸¿"I?½å—UéãÖ?«¸¿"I?äÉì~(?¹DR×àžˆ?Öl'ű?¹DR×àžˆAGN3FGL J2139.5+3919@UÐ?'æFñÀ#бx³pÀ9›ó÷´$À;}ý¬h©?ð¥\ürÖ@+ƶ³/î@ƒ¦¹Ù«¿ëÑâÔ1V¿å'Á³`Œ¿àª­<±¹¿ã>›¥ÂUNASNone@|Ê_ö"FPowerLawnone	?ïìÉJ:?s5Öæ~9?cý7ÒÍÀ?s5Öæ~9?ë«B_1O?'%©TD?ÁRöƒ:ò?'%©TD?ï$pÏÃC®?'Ï",?›qæ'î6?'Ï",?ìA̞ 3?™ØLé¯ßì?½÷›þd?™ØLé¯ßì?ïǜ}¾`'?'HÒ?|1Á:<ÒÇ?'HÒ?Øؤûç0j?Ñ7Uk0>{?㓭'gË?Ñ7Uk0>{?ì´d‹×?§4zôÒu9?º\ß¡GŽ?§4zôÒu9?à¬6ǽCm?¹Ž;Nð?Þ§'p…y&?¹Ž;NðMIXED3FGL J2142.6-2029@?$i@5z5ÀGG@Ý?á—À:å¡Ý4ùÝÀ;Ά"W£?ä¤õ߯lY@
Ö3=o!K?ø[6CÌÞ¿ÜàÃ2f§¿à"ð&½ü¿ïÿƒb½?ïÿH
úƒXUNASNone@Ê5RIº^PowerLawnone?ïæ75»¨?ŸfO,?iÈÊdŠ¿œ?ŸfO,?ïÅ*RÓ¦J?•Šr'Í?}jւïN?•Šr'Í?íÍr¼µþT?¡ƒC¦NÜþ?±"jÛ\?¡ƒC¦NÜþ?ïü
ö?DråêÑ9??§…j'z?DråêÑ9?ï¯Z8«~?>¶Pô(?")`'.Vx?>¶Pô(?îòfEÈûÌ?®&20kè? Ù›¥(C?®&20kè?ë+V‰¾I?®vºô'?ÃR¥ÙÛ«?®vºô'?ïa8,þL?¤Õ¹;'«¨?"Øúc¦?¤Õ¹;'«¨AGN3FGL J2142.7+1957@Rnì€Ç:½À8dv}4ßÀ:±<¼M#À;ÝGP ©Ä¿âjaj©9@
Ü7ùÁx@ÆÿXeG¿î(ÂX¿Þÿhd‡,ô?Æ;4}¸	¿çxšö]UNASNone@°j&éxÔþPowerLawnone?ïþç¸5f?!6Ð1ɀ?!w3Î9?!6Ð1ɀ?ïÁ\má|T?'6z"vp¡?QÉ`?'6z"vp¡?ïÞ1ðײÉ?e–[+¶Æ?pç‰'Û¸?e–[+¶Æ?ïýÊön‡?$$LkƒÌ?1¯Á´
?$$LkƒÌ?ïüK¸÷?@OÒ¾[¦?=§0£n0ö?@OÒ¾[¦?îÓÀ…Qõ&?´Dzø"‡Ô?¢Ã÷§qž?´Dzø"‡Ô?ïœsc~?†	sÓ(´ê?ˆã:ñoMÔ?†	sÓ(´ê?ïóáåv'?X¢)ùD@?X<5óOk?X¢)ùD@AGN3FGL J2144.6-5640@u8}¿HÀFßÓÃa@À:œF&Tþ_À;¹ÌÏQ‹?êÔ¥ý¼?@až½c£@¨j¥§š¿ë'FcM¿ìdG"EL?¸YØxýlÓ¿Æ\Z®î"UNASNone@">\'ÑNPowerLawnone?ïúL'S‰ž?F6£±y¾?FÏa¾Û'µ?F6£±y¾?ï±ÈUœ?–_¾¸;^?ƒÜ´çÌÚ?–_¾¸;^?ïdþ E´"?Š÷M¤¯"†?"`;þ(§y?Š÷M¤¯"†?ïÎ=<mæÛ?g]Ž«õÖÍ?xáaÈ\¦¥?g]Ž«õÖÍ?ïû^Wúÿ?G®lü" ?B† [ãue?G®lü" ?í7Ù¾š&?ÁEìÞ?¶Gq0ÁTN?ÁEìÞ?îZ¹ôFÓ?žäŸ5ìŸ?ªT`¾&ƒÝ?žäŸ5ìŸ?ïe"VïÙu?ßtŸX-:?"Ou Mg?ßtŸX-:AGN3FGL J2144.6+6606@Za¼@ŽÉ@#ˆdüÀ9Óz¬nˆtÀ;ŠÎû{6ÀQ*3d>@7å´™@¤ÿŸÝÖ_¿èz^ò\¿æ¥6û꜖¿ê‰Q"Eä*¿³Ô~.õ…UNASNone@™ò唯OPowerLawnone?ïü•QáI1?FLn¡çŒ?;Ur{?È?FLn¡çŒ?ïÕ/¾µ)?ƒzfHy8?uhs´"'2?ƒzfHy8?ï•<á¨|?'̹Š)?Š°ù‹|ù?'̹Š)?ïÿÿ<"8> ù%%h>˜dáî䇌> ù%%h?ïèJ÷AŒà?qþ†Ýò…?gµ‡y`³?qþ†Ýò…?ï
Á~åä ?°ªlć*˜?žGÐ#C|?°ªlć*˜?7x?žn»KOqž?§gljÿz?žn»KOqž?ïÿÜà|hB>û$ ¤ÜD>ñ¶)Ó>û$ ¤ÜDAGN3FGL J2145.5+1007@Pƒ:'£À?‰Å«âqÀ:žÉã%ÕÀ;ºF"
q?ØøšJŸ@
%Â4‰´?ø××?A‰b¿ïĸ#G'Ë?èF"y&²q?´pUñÍ¿ºî‰FKz
UNASNone@Åü¬‹C•PowerLawnone?ïþëoœ'j?Fê->í?!I5ï•c?Fê->í?ï¢ùó)5Œ?¡žt¬œ£?‡AƒCqë?¡žt¬œ£?ïÚI7µ±?lº½U?rÛd o›?lº½U?ïõ€m¬3ƒ?@dÁþ?Tÿ$ȕ:N?@dÁþ?ïüò³}Ø?8ÌöU1O?8o›'ÇϪ?8ÌöU1O?î‹YõY?·wªƒ??§Oú\Z§t?·wªƒ??ænœ?ƒŸEÆh½?‡ÆSOÍ?ƒŸEÆh½?ïåíˆë1Î?a`)‰±Ý?jwnZ?a`)‰±ÝAGN3FGL J2147.2+4730c@Wnõs}¦Àk¢æIvÀ9"La…VÀ;6É5h—™?ãÓä(^@
Vu´¶@w‹¿ç60¿â(ÙcÅ2‹¿åûhk¤=â¿è¢'ð'ßn¿ïþŠ¿·¡UNASNone@ƒJëIºPowerLawnone8?îû±¾B_:?¢l¤ç? Dä'Ú_?¢l¤ç?ì¸I«xFì?½3M'z´?º=²¤=ȟ?½3M'z´?튀ÏÈ? Vn¾Òø±?³«ùˆ5¦Ò? Vn¾Òø±?ëHÅ°ñƒ?š1?-¶sN?ÂÜé<;'ô?š1?-¶sN?æŒ{}=²,?Éyˆ—"¯ö?Òç	"›¨?Éyˆ—"¯ö?Û×Âìp£y?ÑoØTQ2?â‰Ç®D?ÑoØTQ2?èˆÿˆêRw?´7}œ+?ÍÜÜV¶#?´7}œ+?ÓϊŸß7?¬Ã
)šEK?æ{˜:°e?¬Ã
)šEKMIXED3FGL J2150.5-1754@AѺ^5?}ÀGºCªy»®À9¯[¿PãÀ;¸@p"Í¿¿J‡C3d@\>ø8`o@Evå¿èFì‡'Q¿ìÜìÌéË¿ÜMÓ4<j¿é	¿ônž¼UNASNone@~Ð8†YJõPowerLawnone?ïþœc߉¤?$Š¼Q«?&9Àna
¿?$Š¼Q«?ïÈýZ'Ï~?'0r
¹|
?{R¸xÎ?'0r
¹|
?ïÛž
²?p°¸‹ù{2?ry°Ò«?p°¸‹ù{2?ïñþdõM?DÂzü6Û?\6xZ'I?DÂzü6Û?ïþw$'Hù?* rNz<?(¶âóÁ?* rNz<?ï(F³²?¥®šÖ²3+?šþ~À¨?¥®šÖ²3+?ï£ßZîãù?ƒÖè¤çÿ?‡)N•Õ¹?ƒÖè¤çÿ?ï–ñ=fà+?{R'T('?ŠC°¦Gõ/?{R'T('AGN3FGL J2151.6+4154@V­ó¶E¡ËÀ"åÈ23XóÀ9°ÏS(œÀ;jV9Èxª?ç;™|Ïo¦@(ZÅ4¨?ý"ˆ`Xy?ïÅÛýþYH?Á7†""0ý¿áö7™¿Ñ—ÔtAUNASNone@±÷‹"Ðå`PowerLawnone?ïô?&h??tÄxÎɀU?W´E d?tÄxÎɀU?ï	NÞ4~?«†¹¤Q?^Ö+¨0?«†¹¤Q?ï³K…B'?|Uá¸\t?ƒ;í
Ù`E?|Uá¸\t?îº
X¯«?Š>=tÌþ?¤^OWáPX?Š>=tÌþ?ïÉ>ísø?|°¹Öƒåg?{`‰_ì ?|°¹Öƒåg?ê–V»g?Æ·fm6(?ŧ³ò¥b?Æ·fm6(?îñUoôÈ?—"=á£MÁ? ê©Sxv?—"=á£MÁ?éN~ùK?¸ß&ç?ÊňÒ?¸ß&çAGN3FGL J2153.9+6626@Zž†ƒ<`@"ÚÚUK‹ðÀ9²Š½]ÄÀ;%ôß:›¿Ù]W…3A\@–"t¼@5_®ç4?źÚ
fпàWågÎE¿îÀ°^×ý?¯#³=£‡UNASNone@'­?b¶®}PowerLawnone?ïê
íÿL?tDD$â€p?eæòF:Ã<?tDD$â€p?ïÊ\Ò`Vú?‰ÓGf'&?zіŅ®÷?‰ÓGf'&?î;­ð錡?š­µâ"êÿ?¬E ôÖÑê?š­µâ"êÿ?ïýZö%?,^'6%…?5/w˜³?,^'6%…?îéñº†½ä?¨ÕÓ·›¹å?¡`äV¸:È?¨ÕÓ·›¹å?îÚÙþ
·y?²½c[ƒ¯.?¢R`$ˆv?²½c[ƒ¯.?êûœïÑà?±ªÃ»ë¤?č¼@¸'?±ªÃ»ë¤?ï»mìý"?'öÉBl‹?$¿é¡?'öÉBl‹AGN3FGL J2200.0-6930@tö"Fs'ÀD{ꁺÀ9°Úx†ú[À;À‡»JÄI¿Ýjá€Õ@
µ"}¥ó@Î
Ÿ–2Ý¿éŽýCô¿à7ðeiwy¿éÛ(I+¿ì9Š¹	ªUNASNone@‹<¯hیPowerLawnone?íKmd?´'Oø…?µ¤"Ü[æ$?´'Oø…?ïËg@š¾¡?´TBèÖð?zL_"´3k?´TBèÖð?í]ûé£{? éotó»?µ€! ש? éotó»?ïÔ÷ûÇ«?c^¢¶òo?u"*¸?c^¢¶òo?é–Έ02?Ȟ°ÀãÇ?ɤÅß?7›?Ȟ°ÀãÇ?î±Ö'>"È?³5\`ܗN?¤â–銇?³5\`ܗN?ë™?îÓÓ?ª^"ßñMÓ?Á›G´°²?ª^"ßñMÓ?ì¢_¢
?®È5QZ5?¿7Zíï–?®È5QZ5AGN3FGL J2205.9-4704@uàÛv³¼ÀJ•=êFZÀ:RhDŒ÷ËÀ;ç&p­F?㋖͝"_@
¡rŒÖ@OÀ A¿ì@%"0›v¿çÿ–VKÄ­¿Ô›ã<óå¿ê??\¦
	UNASNone@và.]á\§PowerLawnone?ïû'RˆÁŽ?A¼`Pݦ?Aöµ?A¼`Pݦ?ïa—,µsG?›'˜	òS6?"Íg™É?›'˜	òS6?ïR(0ˤÚ?‹uBêcË&?•ºùèC2Ë?‹uBêcË&?͈‰|?'¸gÌ(?§W#(SO@?'¸gÌ(?ïø$
ÄÄ?TxKKóëj?OoÊ
ªü"?TxKKóëj?è¡w^†H.?Ìî#Û7¯Ö?Íz"…æßH?Ìî#Û7¯Ö?îǍE"só?˜wÄݕ?£‡+©=Ò?˜wÄݕ?èhëÉ3³?»¡?³Ò³t?ώ\PÛ16?»¡?³Ò³tAGN3FGL J2209.0+3652@V5*"8	À.ûBªŸ{[À9Ýã‹U38À;ª€÷â$M?Ä*½ðs@
¦zÐ֜¯@±Ø@žUÁ¿éùö˛@Û¿íÈnµ%¢¿É$ŒÅSd_¿ß&Yÿ»UNASNone@v[3:}ªPowerLawnone?ïÿhE}|?%2OøLåÕ?òð~J.€?%2OøLåÕ?ï²ö1"?"ÐGéi3Í?ƒB|€qèð?"ÐGéi3Í?ïÚ@ è"?nÔû¨Ù?rßï§2Øq?nÔû¨Ù?ïå{­¨ø»?RQ›J¸z?j"R¢m?RQ›J¸z?ïü*æçê?G2)x°Ây?>¨Ê–¥¦°?G2)x°Ây?îDÌi¿P&?µÃìÜIš?«³9fž²˜?µÃìÜIš?Q\i
?‡»4ƒq7p?‹T«¢"ç?‡»4ƒq7p?ïf–3˜*?†œ@2¸š?"-?>´d¯?†œ@2¸šAGN3FGL J2209.8-0450@K׺Âß
AÀFÇvõ׈À:--U£ "À;eÁsÓ6s?çÒR:èç¾@]ûÞ³)?ôA»¿3\#¿"¨ÚúîæV¿ã¾6ÿæX(këÔ?¶÷›CÈÆUNASNone@يÌ9XbPowerLawnone?ï÷Ãoo¾C?`^Ŧ‡?Py!mzº+?`^Ŧ‡?ï·ÏZyP×?"T	Âvˆ?')qÑô?"T	Âvˆ?í»
ïÏ'½?¤…ÚÍzùo?²'†Â?¤…ÚÍzùo?ïí¯©Yâ?U¿Îeø\?bPV æ`?U¿Îeø\?ïã¸o®Ê¿?tcý'ùÚ§?lGZÔ(‹?tcý'ùÚ§?îŽÄØó<?·$4¤JÃ5?§²{C?·$4¤JÃ5?ít0BàFÊ?§ý>	Êü?´^}èýÉ´?§ý>	Êü?ïPs<=?–è/ÙÖ?•ýq¢ˆ\?–è/ÙÖAGN3FGL J2210.1+5925@YëäO QD@Àc'†WÀ8œzšÐÑ>À:æRxrØe?ìÌ;5œUG@0–Jښ@üVàŒr?¿á¸VCT¿éF'ì‹¿í¤ˆ3{闿îIšt¤±jUNASNone@€X]>Õ'åPowerLawnone?ìŒél£?´trÄá˜?»˜´Ÿâçt?´trÄá˜?速p%àm?Ã0}vMd7?Éý'?h~L?Ã0}vMd7?ë((ˆèÏë?ªârà
?Ã_]Ü\ÀS?ªârà
?è÷Áö™?£T†¤{H?Ïð ø%ɜ?£T†¤{H?ã¹üq?Ê}OÂU?ÙÀŒñÍ?Ê}OÂU?Ӓ´|bÀÙ?Ð4øæíE¤?æ6¥ÁΟ"?Ð4øæíE¤?ãH5GyU?¼-£Íá0?Ùo•q
UË?¼-£Íá0?ÆTQÞ;'?¥2¯-·¢?êz*ëˆq ?¥2¯-·¢MIXED3FGL J2210.1+6043@Z=îx@@AéÿãzŽÀ9Ë…ãpÀ:Ö8Ûé B?ÕÛNt®@gAžÛÍÇ@´ò€e–¿çý%ôËj¿ïÿíb»ÙW?ïüÎδü¿Ñ$|bßUNASNone@²R?åÉPowerLawnone?ïø7zX?lÈS¨I?O#™¢ ?lÈS¨I?ï´
"'lÏ?'na…Ì <?'ü›*(?'na…Ì <?ï,{‹3Ù?–úi\Ýó?špŽ'½Lö?–úi\Ýó?ïû׳ý©?@7ÐûÐ?@¡4"á¼?@7ÐûÐ?ïZž‡?mô
dñ
ú?a|a©æ?mô
dñ
ú?î…]IÝÊ?´"ÖˤÛ?§ª+b.s[?´"ÖˤÛ?îbövá«#?¢œ)D[Ÿo?©Ð˜Q˜Ù?¢œ)D[Ÿo?ïû%kÒê?QHŒHYR?CãjSt
?QHŒHYRAGN3FGL J2210.2+6509@ZÁøL­W¼@–*"Š>À9ƒžòžîmÀ:̍Wk÷ ?Ú¿Ýs–®5@áQ•sð@ϧŬ¿è'+f¾®…¿ëŽ´Ô©˜¿ç""
Ó2¿ÂÆ!{¿'ÑUNASNone@›#'Zîc PowerLawnone?ïíl	h‰?v–£Qʔ6?b"öT'?v–£Qʔ6?ïµi^Æèe?'¿d'Eø?'¥¨F¶ÂÒ?'¿d'Eø?îâ—uŽ3?MW¥!?¨֊^êÑ?MW¥!?ïß¡âØÅ?\ÕÝ«å÷?p/˜¥|?\ÕÝ«å÷?ï10võ?£­jGò?™Ý9ïtsn?£­jGò?íínï]+»?¹^Ãd+>@?°"ˆƒ^Ô(?¹^Ãd+>@?êv7Ý<À?·>·Báw?Æ' ‹é?·>·Báw?îs°ªq?¡ô$UFo?¨Ïôõ_èô?¡ô$UFoAGN3FGL J2215.5+6122@ZV~ùÛ"Ñ@™l?Ä;.À9Ó'YáÀ:Ég¦†é?òíȀþç@
Q[ÅM§~@;¿Ý/ñ¿Ò±kã(þ¿çèFiµ•¿ë…ü~ ¨¿å'ph]¯UNASNone@K=ÈK^PowerLawnone?ìó̗Œ'å?»ú0À»ˆ?¸a›D	\Z?»ú0À»ˆ?á'yì€?Ï\á!Ãt4?Ý÷±&ÿÉ?Ï\á!Ãt4?ë$®*þ¹â?ªœb?É?ÃmGTv?ªœb?É?å›]@G?­6kE#D?ÔÉÑEéq?­6kE#D?܅l­õ"?ÏZTŽ'l"?á½I©6:?ÏZTŽ'l"?¾pyBiºŒ?Ãa_ÇÌîí?ì1ðײȮ?Ãa_ÇÌîí?ã 2n«óþ?ºÙ'ÛxûÙ?Ø¿›"¨?ºÙ'ÛxûÙ?ĸÕîx\ø?²x³ñKÁ¦?êÑʄaèÂ?²x³ñKÁ¦MIXED3FGL J2217.2+6346@Z·#c²W@KpïVd'À92ÀÁ%ϝÀ:ïµk‡7—?ÙÒ
	ª^õ@
>>lLYu@v/ŸTïq¿ÁøÄË)<B¿èîaœýý¿å¨øál…Ô¿ãS'æ&]UNASNone@ =ŒIº^5PowerLawnone?ïÃGU²— ?•~(G?~\U5Òwï?•~(G?ïŽké@?˜È—}K?ŒeÏ^Ù?˜È—}K?î‹n`Zޞ?™(;xöÁ?§Iû-ý!?™(;xöÁ?ïAÙÌÌ?wë×W~çÉ?—ÄÆzœ"?wë×W~çÉ?ëƇÜ,ç?Â;žZ'>?ÀåàLc±?Â;žZ'>?ì0>ÒJK?Á?rv)õ?¾~1m­¥?Á?rv)õ?é¦Gc''ó?»µ"OúØè?Éfâsc`3?»µ"OúØè?é  Kºhœ?±ž4­uˆ\?Ë}~Ñ]?±ž4­uˆ\AGN3FGL J2217.8+3207@V3RÒ4ëšÀ4_¢œwškÀ:Jß72œ4À;Æ|°TÇ¿ê©ù>a˜@¬Äĕ›³@(_o§-¿åØû)xí¿åÛr…¿®<¿æcY·_ü¿â*Ûì'þ*UNASNone@`$¨ÁTÊPowerLawnone?ïèè/ît?¦à@VŽ*p?gÏë_ï?¦à@VŽ*p?ïÅÐ
–bû?g;ߐZ?}ù 0Ú»?g;ߐZ?˜E9N?ˆ';Û­£,?Ñ™õäŠ?ˆ';Û­£,?ïü~™?0­/6T±Š??ÜVe½?0­/6T±Š?ïÑX/Ê{—?†àUærƒ?wSè'¨M?†àUærƒ?îçkY%á?±Í¾ìγ?¡‰OÆþô?±Í¾ìγ?î'1Üwo? `Pàˆº?§ÜãÈÌ>? `Pàˆº?ïšÅþýK›?"®3Ù.?‰N€9Íá]?"®3Ù.AGN3FGL J2220.6-6833@t»ƒÏ,ùÀE~s>»ýrÀ:p'Á—åÀ;úIŽ¿K?Á3ÎCoks@UQŽ&ô@
`V,?¼ôty­¹¿¿#H¼SÐ.¿ä­>!MØ{¿âiØd
NPUNASNone@£5¹™™™šPowerLawnone?ïüÊ[áÛ°?8Ó¢)¨ŽÑ?9­ 	#Eh?8Ó¢)¨ŽÑ?ïË_¹ÆW4?ñÌL''?zP#"Þ?ñÌL''?ï°õå0,)?}ºÕÖ2Þ?ƒÂ†¤&ÁÝ?}ºÕÖ2Þ?ïßë<pëó?S¬æ`›C?p
aè†Fk?S¬æ`›C?ïù´^Á×P?Jéé´i'?I.…b0W?Jéé´i'?ï1¥¿l½?±EÉnæ–?ŸyËM9Ò[?±EÉnæ–?ïiq5w[+?ë3º?'ÑÙM¤þœ?ë3º?îÌTá?©Á®+d?£:¾F;"?©Á®+dAGN3FGL J2223.3+0103@PMÔA5TvÀFL\|ؙÀ:>}—ÛSxÀ;­?)
»E?ÌÀ™~§â@
Ñìšó`à?üðxá=G3?ŗÊeÙ˜¿á½'œ¹Î¿¯"ç<Ü÷Š¿Þçg¾çB*UNASNone@°uXbMÓPowerLawnone?ïÿ+5Û%¢?!ƒE{úk?™?­k¡?!ƒE{úk?ï»jF)Ê?—VêðXä?%~®Íƒ?—VêðXä?ïß%CÓ¶Ã?cQð_ég•?pm^Efh?cQð_ég•?ïîä´Êøa?FR…—?aKBƝ?FR…—?ïýò-&C?1ô›"ª?0oJÀy|?1ô›"ª?îζ  Øy?µ!Ž®a°R?£–=ûl?µ!Ž®a°R?ﵧ
w'?'OíáÁçÇ?'– Bá–#?'OíáÁçÇ?ïĺ¡žS?p•c	Õ¸Ï?}¢ÿ6>?p•c	Õ¸ÏAGN3FGL J2224.4+0351@QšmÚÏÀEsG0@9¬À:sˆ¾€À;§¤&»U¬¿É'6G~ˆ‹@HtÓ¼€#?ù‡µ'm,?ïü6Ìq'¿àà~~ú˧¿áÿx÷žÄ?Ĩ0A\ŽUNASNone@€0£×
=PowerLawnone?ïÿCš3f?õ rù?Œ¶º*qC?õ rù?ïºÁ(÷'?žðü³Ã‡?OµÃ›s­?žðü³Ã‡?ïń–I¥]?xå' Â?}=´Ü)Š?xå' Â?ïþ"¼"Ú?V¦
d?'´9eS­?V¦
d?ïþ>_iЇ?0"GPýu?,D¸¾'?0"GPýu?îã3£ÄQ?µc\·¢)q?¡Ìϗ{ˆí?µc\·¢)q?ïd"""D?Ž¯ÑEUÀ>?"
Ý‰?Ž¯ÑEUÀ>?ïñ±LÏÎ?]âé1òíN?]ƝéÅ@?]âé1òíNAGN3FGL J2228.5-1636@Ew}XÀK®ðà¨KäÀ:&êÓ²šÀ;¾Îf*…?ã'ó¬Nkã@<k›"€X@
Y ,Æ2¿ê£Oÿ'蹿äDn[¿å^gæ‡ø¡¿Ú·ï-}oJUNASNone@‹'ÖÕϪÎPowerLawnone?ïþí€mðì?"Vªò û†?!'ü<ý&ï?"Vªò û†?ï¾Ìx¶l†?'þ'ñDL÷?€LáÈn¬?'þ'ñDL÷?ï°ªÿêÓÀ?|TåEЪä?ƒÕ@Ûsð?|TåEЪä?﷗ýñ²?gPŒ!}~?'³4o{?gPŒ!}~?ïü…÷Ï?C†*J>Á±??‹ÒåV?C†*J>Á±?îŒÿD™7?°%'2Ëmø?§0¹C?°%'2Ëmø?îtT
tÛ? òú"hM?¨º¿,päS? òú"hM?íÎaBÌ>™? ‰ӄG?±Œõçæ==? ‰ӄGAGN3FGL J2229.1+2255@UB>ÕÀ=FژgjrÀ:9^>y¸SÀ;ÊPg÷`¿ÎnÝ	@Oðò'@é®@o±¿¿åüCà‡¿ãù!3¶¿és¤¦©M¿®µÎCõl6UNASNone@›ûN¤¨ÁUPowerLawnone?ïý«ÊÒ)a?7sÙ«Œq?2¡«†+Jû?7sÙ«Œq?ïÈæ˜rI–?½µÅ?{Œ³ÌZ•?½µÅ?ïÂcÇûÁ?n³#*Áèu?~Îà'ó©?n³#*Áèu?ïýšEC´"?%\›qíüp?3-ÖUÎDò?%\›qíüp?ïóÃIý`O?`ÀbAyÙ?Xyk‰sK?`ÀbAyÙ?ï#'MÂM?±Äk&ÛJ?Ÿ»o W?±Äk&ÛJ?ï&E+$¾H?"Ÿ›Œ²?›7Z"ˆÿ?"Ÿ›Œ²?ïӍ>Ӌ"?s¥'IàŽ?v9`³ÆÙÕ?s¥'IàŽAGN3FGL J2237.5-8326@s3"µÜÆ?À@DÈ`VíÀ9¥"L["fÀ;6dÃÎ÷?àŸñgêR¢@¾æåÒ­7@x4€3>¿çð¥ë>.¿â5v{Ô¯¿æûFf…‰Ü¿îVP.@°UNASNone@–¨Ô•*™PowerLawnone?ìÛ.Åi*?¸áèò*&?¹&‰Ù<"±?¸áèò*&?ï¤tNb?'VÕù¶?†øböÆû?'VÕù¶?ì¿w_ï(?¤lž2l¿?ºE‡†¿?¤lž2l¿?îÇØò¨‡&?—¯''
×?£'pÒãئ?—¯''
×?çe¡@Ƴr?È°dt§Om?Ñ4½~r™?È°dt§Om?ìþTëP?Á;†q|Lµ?¿@
X¥ù?Á;†q|Lµ?æ܈d?¹JÒ?H,y?ÒGÊïÒá9?¹JÒ?H,y?æ(±ËQ"?²îhkuÛ)?Ó®œiÇ]¼?²îhkuÛ)AGN3FGL J2244.6+2503@Vpڐî¢À=ˆb¡µÇÎÀ:§x+ŠÈÀ;æ<³åu?éÉÇè?!²@
Õíðˆéž?þ¶1_žv"?Ü*Ž'?µO˜©
¤¿ÕQ:í^45¿à¢Ou´7UNASNone@©ÿíVPowerLawnone?ïþžô!z?$w÷cäÆJ?&ö,;.¨?$w÷cäÆJ?ïÖ³Å-¶?"Tpg« ?‹ÊSÕZ'?"Tpg« ?ï×èȒÊ?nr´T:QÑ?t›É…~´?nr´T:QÑ?ï'ˆùŸyê?y$Áui°;?›àÌÂÎ?y$Áui°;?ïü*€å¡8??'U"ñx?>«ùR[·??'U"ñx?í¸‰h–cÒ?¹CYh26?²;´¼–»ò?¹CYh26?ï±O€Vf?ƒZÒç?ƒ¬ 
à¤]?ƒZÒç?í;™ð<Ð? Zp$Zq?·Î#/¢2"? Zp$ZqAGN3FGL J2247.2-0004@QÂÀð ÀHÞbäѦÀ9åóìÌÀ;›z6'?Ëøòd•x@	E—丧@Ü·àð?¿b v°¿æûÒp¥¿àÞ+ÿ7X¿à,_ÃEJÉUNASNone@˜yzCþ\'PowerLawnone?ïÿÞÈ3? Œ±vù ?d"Úœç? Œ±vù ?ï½Öy7¾!?"¾~ÖÀ?€ŠaÂ损?"¾~ÖÀ?ï܎Ó0ØÕ?ni¯'À–º?q¸–eƒÑª?ni¯'À–º?ïÛÜ^)ï?UÐЇ}?rÐØå$Ù?UÐЇ}?ïýòé¹d?4g™™K)?0h²—Õ?4g™™K)?îÓ8P^Z?³Y2_†tå?¢Ìzý®3]?³Y2_†tå?ïŸtEæØÖ?‡›ˆ¬îR\?ˆ"î†IÊh?‡›ˆ¬îR\?îô0N&~š?‹ë÷]º³T? ¼û(zg?‹ë÷]º³TAGN3FGL J2249.3-5943@tqŒ½D¦ÀI¥¶…ì>À:åwo£&
À<'Y
]QÀè>WÔ}E@
ŠÓÒO˜š@dhÀí_¿æ;Ïl—á¿ÖËÑǀ¿êêu'°"S?ÈKÕI%ÁcUNASNone@ w<í'hsPowerLawnone?ï~÷°Œ`‡?¹ÏËàJ?!	ð+½?¹ÏËàJ?ïÖ+Õ¾/s?Š@Ž•£y?têxªÄ?Š@Ž•£y?îìŽd‡>?—/°ï7
!?¡?—oZ?—/°ï7
!?ïÿÿ9å³>k'>î'>˜È-ÈÍÃU>k'>î'?ï`®¸Üø5?¥NGøÇdt?"ê(ë@1G?¥NGøÇdt?ïJ§¶v?¯U"žÇ?–«Á¡P?¯U"žÇ?íÕò±2Š?¥J­1ؾh?±Plvk±?¥J­1ؾh?ïÿØʀ>ÿgpÏ+>óýhó‰ø¼>ÿgpÏ+AGN3FGL J2250.3+1747@U–ª:э&ÀB*R¤ À95Õ"äFÀ:ë°Š`A¿×¡³†!9-@ݽ=¸@@H)`vP¿ê¹ý¯:7+¿æ~@–âÉÓ¿îìbïŽmÁ?á8¶ªCUNASNone@‡ ýÞ½PowerLawnone?ïÿÀ/¥V?	å5g/>ÿèmŸÌá?	å5g/?ïÍTޘk
?ŽÉÃÅ÷wo?yU¡<—?ŽÉÃÅ÷wo?ï~£Q±×?Œ"5¢;c4?+•Îì‰A?Œ"5¢;c4?ïÿô!O…ú>ÖÁÝR¾>×½Á£G>ÖÁÝR¾?ïÿU߉F?'–_Dq ?]œ&k'ù?'–_Dq ?ï''?4ô?²S/qV¢?›»ˆýv?²S/qV¢?î²aÔ'×W? ü(ÕÃ2É?¤ÙâºîՖ? ü(ÕÃ2É?ïÿQ"Tq?ì'h/µ?݂jáÀ?ì'h/µAGN3FGL J2250.6+3308@WêÝëÙÀ7AÐúX÷À9ø8¢Þ¼¹À;Åß3מ?ó3¥^sÓ·@
êr$4¾@ÕãÿÄEë?ÜdR5¾)¿æ>k‹nó¿éΏ¿Q¿ïÿÙUNASNone@‰ ­«ŸU›PowerLawnone?èöޓɠó?Ê[n!?Ì$…°Ù|3?Ê[n!?Оìrb&?Ê®és1â?ç÷0‰ÆÎí?Ê®és1â?çƒá·ü—Q?±-Pšµ?Ðø<Ñ^?±-Pšµ?Úi§7¼Û?©HiȒù?âËx¬d!"?©HiȒù?âÉNØLª?Ò¨B½‰+?ÚmbOf«Â?Ò¨B½‰+?¶š÷íàð?Á»FE<RÊ?í,¡´…r?Á»FE<RÊ?Þ9Âl\Ü?¼Y
ê8?àãyžÉђ?¼Y
ê8?®Jü¾x?Õ>bŠ?îP?ªÝ0?Õ>bŠMIXED3FGL J2253.1-1237@K\bõ˜ñÀMb"aùðÀ:$tÎÀ;ÖËÒÑɌ?îy‡ôom@¥Ô/^@‰åÿά̿ØeöÕ¿èud¤«µ¿ç1ÉÓ7
ø¿ïÁRÿx¾UNASNone@ˆ?'RT`ªPowerLawnone?ïQӕ­–?©A©æÀTI?•ÝE†kW?©A©æÀTI?ëݦèrÖÈ?ÁžW×ön?À‰d^4¤ß?ÁžW×ön?í–Òe¿}? >ÙÍ?³IlØsޚ? >ÙÍ?é"Ãuq1?£-îì*ŒÑ?Ëtò+';=?£-îì*ŒÑ?W?¬¾Òn?¦>þâa?¬¾Òn?ß.Þóž{^?Òë_fMˆ?àh†0ÂQ?Òë_fMˆ?ê¡éS"¾?±¨´­ç?ÅxZ³ïu?±¨´­ç?ѹº.ÜÚ?¯ÜÝÒèM?ç#w¢è'"?¯ÜÝÒèMMIXED3FGL J2254.1+6229@[v"8…
@ ݂ýuâÀ8ÈI°M:EÀ;Gckà#?ÜÉhÚ	 e@A⹞ß@}_Ò"¢¿áßZËuU¿éö¾á¿é#Y…ú¢À¿ç§2ŋKUNASNone@{KC•PowerLawnone?ïöNÅjê?W4gPÊ/}?ScØ@ðu?W4gPÊ/}?ã"µÉ?•z46ƒî¹?ŒÓ‡-¹á?•z46ƒî¹?ï&hLD§$?"9QwšTû?›2öy"é€?"9QwšTû?ïHÙL%â,?ué_®R ?–äÖtd'–?ué_®R ?ï8Áì£?œOòXeû?˜çßµ£3£?œOòXeû?ì4gzHé?Á3gqºh­?¾\Ô-¸º?Á3gqºh­?뾝 Pœ>?²m å$?Á‹~½?²m å$?é4].8?¯&âÁüpF?Ë.‹G‹Å?¯&âÁüpFAGN3FGL J2254.6+4253@YM†DR?hÀ."'›ØÀ9µr҅srÀ;"=?%¯½?àFqï0¤ã@ލz&@FHö…X¿æ]ÓèŸç¿ç`XUŠ(Á¿éèx'{M‡¿ïÿ–ȦCîUNASNone@|±áä÷eþPowerLawnone?ïï"Ú0ý=?cù¨ðÖÃ?`k%')ː?cù¨ðÖÃ?îéšì]"c?©¾½<!t?¡fQ;އÈ?©¾½<!t?ï:Æ~:SÊ?…\"P
?˜§06ý¸À?…\"P
?íW'$&È?ÕÇPW?µG#p(¤<?ÕÇPW?ï€nT=ç9?"Åí¥–o?äjßX%í?"Åí¥–o?棾-5?Ðä2þÁ?Óü¸ƒ¥Í–?Ðä2þÁ?íºyËÈëÂ?£T'[?ha?²,1 Óõ?£T'[?ha?Ûzت6Ûð?±©˜Lã??âB"ªä'?±©˜Lã?MIXED3FGL J2258.2-3645@8R÷ô˜ÄÀP$³=¯ŽÀ:¿Â"À;ïìì'(¿²œN˜lÝ@29Ÿˆñ×?ÿKA¿½ð'¿ãá•5¶C?Àe[é«f¿îÃnšµ?è«é‡ˆÊUNASNone@¦£ž5?|îPowerLawnone?ïøx>EW?ZÒ1Ît»À?Nó¸|ײ?ZÒ1Ît»À?ïÛ^üËÔ;?‰™ðã)€?rP¯cvš?‰™ðã)€?îãaçÚ!þ?•ƒa´?¡Éဦ*?•ƒa´?ïÿ¤™¹
?!Òi»?+hÁ Š?!Òi»?ïÍ©Ò²ûü?'è…&ÓMú?y+ˆEqï?'è…&ÓMú?ïzö5eŽ?¡I'ké+T?¡9W+äI?¡I'ké+T?í0Gyù?¦ç£-e@?´}Å6?¦ç£-e@?ïââ_ÊÛ?|\"g¼¨?mñÓ]?|\"g¼¨AGN3FGL J2258.8+2437@W.~ùÛ"ÑÀ?­W¼xÀ:ÈB#'À;š‰;}"¿ñœÝø©Ê@¥n‰ }9@xO #¶é¿ä¶_ ˆÿ¿îŽ:üçX?ÌÕp'î¿çQù¶©UNASNone@'s×ÜPowerLawnone?ïÿ›Sƒ	à?=çêðßÉ?	+0!°¿­?=çêðßÉ?ïПöç
Ò?Š®´tx?w°n<‡:?Š®´tx?ïårâ¼x?n­&mÖ?jòêiP?n­&mÖ?ïÿÐ9Ã>óàԕb>÷ãp?ƒË—>óàԕb?ïÿƋânA?W™
¾5>üº!q'?W™
¾5?ï0_†Ïp?°ß%—æ§o?™ônCÿ?°ß%—æ§o?ïÎ.ˉD§?z-&³¸?xèš$T×?z-&³¸?ïÿ! "¨¢?íÂ7EÞ?Ûçø½…Æ?íÂ7EÞAGN3FGL J2259.9-1553@IXÜìÀNëD$>ûÀ:O&ËEäÀ;ãpûÞ´?çrÝæƒ4Ü@&î'm¦!@å®À>•¿ÞÏ
Ž¿à>íÚ?¿â"%¸«¿è*‡= UNASNone@™RK]ÌcñPowerLawnone?ïýìŒR*½?.üAùË?0›œ6ÃÅ?.üAùË?ï€)="Á?˜óùȔ•	?õ°º«3¶?˜óùȔ•	?ïÃò§Á"N?y™SX¦
?~¬,ôHÊ?y™SX¦
?î]ŽÒÀ'?‡Z?®Å?ª'Ó¯Þã?‡Z?®Å?ïô h«:+?]y[Co,?W¿.Îz:?]y[Co,?녿"\=?ij/óôÀ?ÁéîÃ?ij/óôÀ?îèÄî˜4Ñ?š~£ù§e?¡s±È5í?š~£ù§e?æmH\²ç?°ß-ñ—W?Ó%oF›2?°ß-ñ—WAGN3FGL J2300.0+4053@YO‰ 'RTÀ1>%Øם
À:5D…kÀ;®ÖuÂú¼ÀøBÃIs@¹®@ð‹?ø9	Ü¿ïØfNq/Ì?îßë5v7¿ìÕ&sÃW?éV¸MäºTUNASNone@ÊIšáG®PowerLawnone?ïöý'U?\¹n&:?Sð}?¶A?\¹n&:?ïËîROûb?Š—òAÔËD?zÖâQ"Å?Š—òAÔËD?ï-"c?•¤‡ºa?ŸÚM™<?•¤‡ºa?ïÿÿì"Â<>€Ä­(·5>d!6B9>€Ä­(·5?ïÆÃßÏo%?|±s•¬?|ž,6)‰?|±s•¬?ïܺfÔÜ?¯Ø¸51?¤h±m–t?¯Ø¸51?î9˜"þÐ? ¦ñüõ!?¬fåä,? ¦ñüõ!?ïÿúrç>Ýzß&®õ>Æ5q_*Á>Ýzß&®õAGN3FGL J2300.1-3547@…Ø=CWnÀP66ŸÏ=ÀÀ:Iæ¯ÌâÀ;ðXr‡ÜÙ¿æ
zßwÓ@FEêE¾@z7?‡Ts?çh\eþÚ¿æpÙquä¿ãlŠ2¿â…f®'+`UNASNone@—öZ¬1PowerLawnone?ïÿAMʅ—?1òVÅq?Ö>ÖFy?1òVÅq?ïܝ­ØôV?‡D³~Á'Ý?q±)-¢ÜÙ?‡D³~Á'Ý?ï¯ûÏÞhð?†	ß%4¯ï?"ú§T?†	ß%4¯ï?ïþSLÙ!š?['ÃfÒw?*Ë20SÉ1?['ÃfÒw?ïÿŽ$4VŽ?i–œ*A?vù¶:šF?i–œ*A?ï}{S»òh?¡m8õÞÍ?P•ê­?¡m8õÞÍ?ïŠa âkÎ?Œ8ÙQ¶?g—¹¦œ?Œ8ÙQ¶?ïï®g›?W²ë͵O?`QíǼí/?W²ë͵OAGN3FGL J2303.7+5555@[
…Æ}þÀÃ@&`¼ÙÀ:@»â™½¬À;œÜD9õ?è»[.ò(@
Z[k5®?ü‰Ÿ¦xû¿Ü1튩ß?ïû­9ÙH¿×þ}êªr¿ä
4Ô?>UNASNone@¼':áG®PowerLawnone?ïýÚÀ51?1nPéz?1/ÂSöU?1nPéz?îQàم?µúD_Û{Ê?®áòg«?µúD_Û{Ê?ïÈNsê¢?vå°,²Ø[?{ظ;îò?vå°,²Ø[?í•h³Xï?•ëˆSêñ?³WLºÓ,?•ëˆSêñ?ïíäNô"Í?c‰oŽ°íÖ?b°ê~ó€?c‰oŽ°íÖ?çk} Ò?ÍX§\¶ö]?Ñ)Òý¾\?ÍX§\¶ö]?ïv÷YNŒ?Œìïh>i?'!×æKó?Œìïh>i?梗±¯\q?·8ßÅ®é?ҺМ¡G?·8ßÅ®éAGN3FGL J2305.8+1658@Vqn?x»ÔÀC€¡UO¾À9Ø+{¯À;Aù¬ÿ§ë?҇‹-ŸÝ@´l8~L@3Œ¼¿éÌý°U®ï¿ì5 æO¿Úæ`æ¹vȿ纕KÅêõUNASNone@††Âø7´¢PowerLawnone?ïÿ°ÏÁí?:¶?ÌÊZÇ?:¶?ïÈ—Ky?'"ÁIŠ-X?{ð´jû«m?'"ÁIŠ-X?ïµ‹?]؍ñªÝ¦?aawè¤ï?]؍ñªÝ¦?ïìɒŽ@(?G¥&úBŒO?c6mºØ?G¥&úBŒO?ïÿÎ4‰}>ú çÂit>øå¹¥È
Ä>ú çÂit?ïOä¢_?²‹öÅæöç?Ÿö#'?²‹öÅæöç?ïÏò…‡Ø–?|F±ü?x½+••3?|F±ü?ï£U×;Õ]?x
l_5¯ä?‡*Š>ɬ?x
l_5¯äAGN3FGL J2309.0+5428@[}VlôÀÚüGä› À:Ž¯à,üÀ;¯§Í9WÀ:$¾ü*@<9·[ÌZ?û('¿/«>?ïÿ/FOÖ¾¿áî$gà±S¿ê+ÛjjN?Î_É4
UNASNone@Æƶ‡+PowerLawnone?ïû\ÛßJ?Ié61P,ž?BŒ'-ÏÝ?Ié61P,ž?ï¿ÁžÆT8?«""±}Z?€˜L³$?«""±}Z?ïIy¦_$Ô?ªH.5b?–ÐË0«É'?ªH.5b?ïÿÿg‡VT>˜ ãQ|iú>"9æn>˜ ãQ|iú?ïâ,.ÿiO?qOûyCo?mÓÐê™1"?qOûyCo?î©éqâà#?³"¯ª6¦®?¥ahàöÌ?³"¯ª6¦®?îA¤CÒÏ? ©fpkZ¾?«ïÀV
? ©fpkZ¾?ïÿà~–š?&b1×â>TË?&b1×âAGN3FGL J2313.1+3935@YÃxFÜ]À3uº² À9úò03¤rÀ;º7'´yð¿îñØ@I·yS~@Xk 7™¿éD©Qü¿êÀ›ñ¸"‡¿æPü¸*†ð¿Ô¢[oéUNASNone@xYÈó#PowerLawnone?ïÿz.ÍÑb?¾d¨hWÉ?º-=¬¹$?¾d¨hWÉ?ïËp2åQö?ŠZôQÒÙÍ?zGæ­£X·?ŠZôQÒÙÍ?ïÚ.§³7Ð?h"Ï[ôý«?rè¬wœ?h"Ï[ôý«?ïÿ¾Ðq]>ñÓÈ?¢?Kðãê5>ñÓÈ?¢?ïÿüìú?!±-»d´í?€]§€þ2?!±-»d´í?ï@Ÿ÷h?¯º"^h?·îQ(|ü?¯º"^h?ï«°[쩦?{?B^j?…è÷&¢?{?B^j?ïü	þª7?9³"cЇ‰??·ñ¨ßó?9³"cЇ‰AGN3FGL J2318.6-3829@vKÂã>ÿÀPáú~¶¿DÀ:Cê¡ô²À;úWâ?$Ù¿â"D‡»Ã@
Ò9u—‡@¡ß¹8›¿ã_'»Ëj¿áÑ)¨<l¿ásŠƒH–¿¿ïÿúw2šUNASNone@]/O
"MPowerLawnone?ï¢f4šïä?¥¬ÝÙÜ?‡frçw?¥¬ÝÙÜ?ïЁ9rß¾?Œ·óÜ7!J?w¿cNE?Œ·óÜ7!J?ì™OœËR?¤µb‰ùBÀ?¹ë5ƒ¥n?¤µb‰ùBÀ?ïìOAÙ´?RíR¹ÃS$?c°¾íÇ´V?RíR¹ÃS$?ïÓYq
"=?'l—÷»µd?vSGƒ¬Ý@?'l—÷»µd?ï0ÌH?²-1Äü§?Ÿ]=àÅ®õ?²-1Äü§?ëÐÓM€¢Ž?«ñÏ«óe?À¼²ÉýuÈ?«ñÏ«óe?î¶C¾I?™Ý+ÄÈÕ?¤›ÏñÐn?™Ý+ÄÈÕAGN3FGL J2321.3+5113@[7ÙÓEŒÒÀ"Yò™0À:ƒ¯'R£;À;Åú¬(©¿òSdvL7'@
XÕȞê¼@&ˆ "ä¿âm
&õbB¿ç¡˜Á'l¿ÇÏÿc-f¿áÅÐÚ#UNASNone@®ÑÛÚQÎPowerLawnone?ïý¶H?Α?]'¤7?2M»þù.ö?]'¤7?ï—ª´§›?Ž‹È>«]þ?~´*µzfŸ?Ž‹È>«]þ?ïä—Ö á?q¢ tÆMÇ?kæheØ> ?q¢ tÆMÇ?ïÿ»ê|`#>ô"!{Ö?Y6…P4>ô"!{Ö?ïþe ɬº?)LÙM+JÙ?)­ó4Ósx?)LÙM+JÙ?î¶Ä™'Oã?³Ý-jŒßÏ?¤"¶i~¶Ï?³Ý-jŒßÏ?ïÛ©êÂ8?yDü:&ƒ?r+ÛsÜ?yDü:&ƒ?ïý6ݕO'?4AWtS¼?6IÂ]+?4AWtS¼AGN3FGL J2321.6-1619@KßÕÃÀP¤yèQÀ:Óe
 ÒsÀ;ÕSV¿)v¿;oX» …@
H€´ãw?ø†D 
é¿ïÿG+À^?ïÜèêi?à_ÝKRÂM¿âI:0¨iUNASNone@ÁíÕ?|í'PowerLawnone?ïþ"%oö?3év+€>5?&½©rÅdb?3év+€>5?ïÐ)7À©?'-½z	át?wëdvþã@?'-½z	át?ïžD¹˜g•?ˆÂ>'PÃê?ˆnш¸¾?ˆÂ>'PÃê?ïø§Ð$V]?AEV90Aù?M`¾bëdÝ?AEV90Aù?ïýqٝPï?8YÏúࣝ?4q1êgS?8YÏúࣝ?ïP'æò	j?¤ÖÐÏÄV?•ï£&æ<Ã?¤ÖÐÏÄV?ï\µ"µ?'IéÇɬ?"iMqXúñ?'IéÇɬ?ïñú<WÛD?b¿ÂéB?\‡UÈ×?b¿ÂéBAGN3FGL J2323.7+2523@XÇP%"õÀ@²õýG¾ÛÀ:{—)|ÑÀ;â%™È"¿å=äiÌwg@gGPvÿ@__¶ôÉ¿è?+~UgÞ¿Ü«'GËú¿Þ"ZT®ä¿â1@1ôDUNASNone@ #S÷ÎÙPowerLawnone?ïÿ¿r""?µ'ìÛÐ?…Uj?µ'ìÛÐ?ïÏr칖?ŒNŒE—:¤?xFñ¥ Û?ŒNŒE—:¤?ïäÇÁäÖ?s:QŒ›ù€?k8>=…û
?s:QŒ›ù€?ïþÓnß?)ӈ™Kè?"Éh¨œÅ?)ӈ™Kè?ïÿw;ö¦:?À!8¯Dç?y«yn±?À!8¯Dç?ï/Äu²¬?±+ N°æ?šqBËG5?±+ N°æ?ïÝ ë%0?x;''Ø?q/Š_©ƒ©?x;''Ø?ïóº›XÜ?PhêÓ/«×?XŠÈä"xu?PhêÓ/«×AGN3FGL J2327.2-4130@uºü"µÜÆÀP㦠YŸÀ:LÚ")=À;¬sWæpã?Áa^68˜š@µîŒ:5†@4Ý ·0¿ä¬ÍlÍ¿äºà恡"¿ë1pΧËê¿àØ-ÚóoéUNASNone@"¶£n.²PowerLawnone?ïê[ˆ3b%?—×¼äù?e¤wÉÞ+?—×¼äù?ïÂþ—¶H?"n°¨I?~€¹A3_×?"n°¨I?ïsÈØ)*?"óIîs?Ÿ±†ãCÃ?"óIîs?喇t+º³?qi˜ #F?†Ý"õSS?qi˜ #F?ï¥ԙlE?}""òÍ?†¸ÊÒŶã?}""òÍ?íKÖӃB?¿í–	ñ›?µ§IG¬õ?¿í–	ñ›?í-ïC,?¥™½í?¶—†Ã¥?¥™½í?é¤ûSŒ³Ç?¹7"u3øo?Él±Í0å?¹7"u3øoAGN3FGL J2329.8+6102@\M¶°_¯¿Òê~8•À9®ç¸5À;D
ð
­¿ç²9´¾@
:EÌ@|y ç¿è`ÎۚƿålMPjх¿ÇR!ïدH¿â¯3ŒUNASNone@®ñ>vÈ´9PowerLawnone?ïþtÌ-?2"û+ŠÑö?/¸ÀÑôŠ?2"û+ŠÑö?ï¹Jqñ½{?'oœ§?­c'VóB?'oœ§?ïÄɍt"Ÿ?€H:H©¦¨?}›9&É4À?€H:H©¦¨?ïþ"RÃÏ×? ¨LUD
'?-ÚÕ8Øø? ¨LUD
'?ïú]¹W?I…r
»W
?G'ˆÿ—
ž?I…r
»W
?îqùê­!?¶.;¥{,Ð?¨ànÔÄÉæ?¶.;¥{,Ð?ï'9Ò?ŒÆ¼ï2s?‹¼ÛûÚO™?ŒÆ¼ï2s?ïîõyœ×š?Y°Vï*è²?a
†žA­u?Y°Vï*è²AGN3FGL J2331.9-1609@MÒR'ƒÓ_ÀQ$GÃ
0jÀ:5õáõSÀ;ç"6Æf?íEförý<@%Ƃýk@SÐ@Ô?éãÁ^¥…¿àK¯"dP¿Þ¥Y¨ŠD´¿ïôÃaû-ïUNASNone@•)µY³Ð}PowerLawnone?îqŽèæˆá?¹]›¶†7³?¨çq—q÷?¹]›¶†7³?î½\]_<ã?¬iÒ¦‡g?¤*:'x|Ú?¬iÒ¦‡g?ìKé›ö§M?¦¶ûOþ+P?½ ³ JŘ?¦¶ûOþ+P?ìË"\!¿?—ŒwÒü:?¹¦ï-ò	?—ŒwÒü:?íÜ¡¶@Ý?¯ïp.Ã?±òLG³?¯ïp.Ã?ëoºj¸?ÅBêË»TÕ?ÂAW§©?ÅBêË»TÕ?ç´Uk±Ô?¸Žtìý?ЗU(ÐW?¸Žtìý?åÆÎî»	+?µÉ[§fN?Ôrb"‰íª?µÉ[§fNAGN3FGL J2333.0-5525@tC"Ðå`BÀM,k΅3±À9Ñï<c]À;ë›
ß½?í·&ÑaBK@
ð»äó	M@Åh`'6¿ÝèTZÓ¾·¿âïM,¿áéBËùày¿ïÿá_¥UNASNone@'š@ƒn˜PowerLawnone?ëWÒh(nš?ÂÃÜtpÑ`? ¶_^E—?ÂÃÜtpÑ`?è0Z¾g"I?ɱÀ:{b?Ï>•aîÝ?ɱÀ:{b?ëƒIï?ò?¨ðkܜù?ÁóîØC8?¨ðkܜù?åW&º˜²?¬±Õô\Á?ÕQû²ŠÎ?¬±Õô\Á?溟˜·?ÎM"Íړà?ҋÈÀΑÉ?ÎM"Íړà?Ö
9Ù€­?Ò½ÚKe"?äùc~?ª?Ò½ÚKe"?â}‰9
sÞ?¾ ZS¹Þ?ÛíëE?¾ ZS¹Þ?ÄÉ睼­?®7Â>Gq*?ê͆ù?®7Â>Gq*MIXED3FGL J2334.4-7948@s1³g ù	ÀBX—{žÀ:OŽR=ºvÀ;ÃÍ¡Þâ?Çâ|_T¬Þ@ºý¡Uü@ø¨™Mn¿è›Ñ¯à'â¿ìitònƒ¿Ð½TÁMh¿æ
åH UUNASNone@"ÚQN;Í6PowerLawnone?ïö~vþd? .Bj€ê?Sò¹¢ü? .Bj€ê?q'7Áý?¨`³I?€›Ÿe°èÑ?¨`³I?ï•ÎôD`?‰MP$a‡z?ŠŒBõÇ7¥?‰MP$a‡z?ï¤Ížr¶?mXd(ö¼?†Ì˜m¡M€?mXd(ö¼?ïýÓħ~#?:x–½I<?1aێ^Q?:x–½I<?휟ªÍ?ºÇzEžù3?³ªs>c?ºÇzEžù3?ï*?ò¼Ô?•ø肷Š?š¸¡†F,?•ø肷Š?í"wGÎåp?§ûb÷Æöt?¶ìEî–?§ûb÷ÆötAGN3FGL J2335.6-2342@DW´ÀR#¶þ.n¨À:PJ›.ÅÀ;Ø*>—ëD¿ñ#†TÃPÍ@×8Ëùh6@-à_PÈ¿åÍ¹¿èy1ÈÇ¿éwíÒ"nŒ¿ß#<*R¹áUNASNone@Äg8~PowerLawnone?ïë?0Âjž?¡á`ê'ÞÙ?dÀÏia"?¡á`ê'ÞÙ?ïÚËU!?‡˜:Z*)0?rš}s	O?‡˜:Z*)0?ïÙªçÜ?—ókɱø&?Ÿ_äÃÃ̏?—ókɱø&?ïþ
ì[ø?$ºY˜·Rî?/Q:ÞÓAð?$ºY˜·Rî?ïëÙpc?s(¹ö›ÿ?do&©º'?s(¹ö›ÿ?ïi¹•kT?¡\ºÄÌ?'ÈÍP姍?¡\ºÄÌ?íÔ£¨¼!Y?¢órU—h?±Zâ¸Õº?¢órU—h?ïƳãÇ»?xÎÌ¥7Å?|¦TAŒ?xÎÌ¥7ÅAGN3FGL J2337.2-8425@s}ŠüÀ@3EbàŸèÀ:v"Z»7À;¬1u¿¾ÚS"´,@
C˜LgŒ¬@ ­`uᄿÔΣUt¿æ;º{ïî¿èì|•å…?ÏwžëUNASNone@©'Ž¤¨ÁUPowerLawnone?ïíVØSéŒ?œ´tó9L?b©'¿TCÅ?œ´tó9L?ïÍ6D"5…?¨Cm?ydݸu€?¨Cm?ï'î¸s¾-?'Ô¥ëš?›(ê©x?'Ô¥ëš?ïû—m	²?6×Tæb4?A¡Âi‰	5?6×Tæb4?ïר@"??~ûIiÚÔí?t+߬h¸?~ûIiÚÔí?ï
ðƨ?±ª¡Æè?žAçC*(?±ª¡Æè?íðƾ¸.}?£>%tk¨>?°yÊöZ?£>%tk¨>?ï‰æ—׫?/·<g›b?¿FdXé'?/·<g›bAGN3FGL J2337.5+4108@[ÓØYÈÉÀ3ž¢	ª£­À:eÉÞÜÀ;Д9ˆŠ?Å+á×¢@@&Ít<"@ÎçßwÊ<¿Ý!.üö=è¿ìÈöÑ$—±?ÙJ»	ÖÃq¿í–©C'ŒUNASNone@™N>Åm\ûPowerLawnone?ïå·¤Ë7?hâ܍šìÛ?jHø_TPÉ?hâ܍šìÛ?ï°ûÊނ?"RPp5;?ƒÿÁ÷Q?"RPp5;?íãÿe?8¿?Kw%:?°àÔNl?Kw%:?ï¿·ˆöfØ?rCk«vÈ?€³Ÿø)?rCk«vÈ?ïЃCŠç?{ìi&Š…a?w¾tHìøÐ?{ìi&Š…a?î=—ÛÜè¬?µ·èšâ?¬&'?À>?µ·èšâ?í§c>=ÓJ?¥ÑÏÞ'§µ?²Äæ
£r/?¥ÑÏÞ'§µ?îûaÐ?¥«êwT5¼? Oÿ»šFÿ?¥«êwT5¼AGN3FGL J2338.7+0251@VsI''>ÀK¢±Ä2ÊXÀ:)>ku™àÀ;Çöåv?â#Œò
Æ_@ÛNšÂ¹y@¡u`F²¿ãÜ©""#2¿çuiÛa²¿êÿw(«¿î.'7$¯UNASNone@ƒ>À//˜PowerLawnone?ïò°°¦?^?Z"~TK¶?Zžž"Æ"ð?Z"~TK¶?҅ÀÁ?•Ý¸¶
e?‰‹T@ûÇ?•Ý¸¶
e?ïPHâòÓó?…|1Ÿwc–?•öã™{»?…|1Ÿwc–?îyeÐ?"IO8Ô09?¦(i¤¶ª?"IO8Ô09?ïñõ•Aù?]îòþÆK?\ÔqˆÁ?]îòþÆK?ì:"ëèEú?ÁÖµG¹ÁÇ?¾.è ½Ð0?ÁÖµG¹ÁÇ?ïŽdîRj?"ugH%Ã?œ®3g]Á?"ugH%Ã?ä¸Ô÷i?³@nݒɚ?֏ßV/?³@nݒɚAGN3FGL J2340.7+3847@[	H˒:À6	zû]À:Ž§©&ÕWÀ;Ô¡¹"ËÝ?°áȚS¡ê@
µp%¬âÍ?þ³ŽÀL¶½¿ë>¿0,¶¿í‡¶	U®?ÞXä¾í!g¿ÜB"Š;,ÒUNASNone@²N?|í'PowerLawnone?ïÿˆž"y?<¤2—|?
Øq‡"·?<¤2—|?ïȘŠ?²G[ r?{÷3–n
±?²G[ r?ïìSã¾?V9Œ>ÃYc?c~¬[z¾z?V9Œ>ÃYc?ïüeM¯Ø?07Hž"??<Փ­ƒý?07Hž"??ïÿ¬Y?;¦tÕ9?ìp§ð?;¦tÕ9?ï̓DÝD?°{'Дݑ?Ÿ&Oœ‹Á‰?°{'Дݑ?ïæ£JûÚ_?l#癷`§?i\µG}ø"?l#癷`§?ïöXÆâõP?U.s­?SNr¸‡?U.s­AGN3FGL J2343.0-4748@t³Ý)4­ÀPY6z—À9áB-¡úÀ;Ü÷'þL?äzZ3I¥Þ@
%}$p@HVßà¥È¿×°֜•‰¿á$ÂÛ:Š¿ãDvcMq¿æç×FÅ®˜UNASNone@"Áb¶®}PowerLawnone@?ïèñöÒÚ®?¥¦?ےVg?g	‡ª<?¥¦?ےVg?ïD'Ô>ž?«ûSÅeU?—{wÂ@?«ûSÅeU?ï¬68jÞ?ƒ %š.m
?"ò\«?ƒ %š.m
?í7CBlX?",îěf?¶Eåíy"}?",îěf?ïÙR1P/?vžP+Ÿ<²?ssÖèÔs?vžP+Ÿ<²?ç<cN4?έ5ÍÂ@?Ñ÷‡9ßc—?έ5ÍÂ@?ï'}-¹]?•.ã,¢?_p>\?•.ã,¢?Þ
'Úëì?¶»Ž]ÿ¤5?àúì9Š
?¶»Ž]ÿ¤5MIXED3FGL J2344.9-5647@t¶®}VmÀM/]»œúÀ:éÊ3•YÀ;÷ÂÅ+?Ç<;±'@W½þ¨¼ø@'3ÀvÓ¿â·Î?ŠüÀ¿êOüÁ¥8¿é'Þ¸©÷'¿ïÿååè=UNASNone@~v±;â.^PowerLawnone?ïùŞ…;¿?Lè…m"Ì?Hé…x·ŸÄ?Lè…m"Ì?ïÆ?'ïC€?oL3ÍFv?|àl#+3¤?oL3ÍFv?ï7aºžæ¤?‰¨é®Ö?™Ȫk]x?‰¨é®Ö?ñ§f{?q'»rÀ
?Y™N?q'»rÀ
?ïýRŠ«.?BÂŪ
šÇ?5k©2íJ	?BÂŪ
šÇ?î5.…¤o6?µÙ|:ԋ_?¬­¦"ó¥?µÙ|:ԋ_?ï
%™&?"÷LyÁ'%?ž]›N–	C?"÷LyÁ'%?êl¿±[W??­¿_™÷(?ÆM:'£?­¿_™÷(AGN3FGL J2351.9-7601@s9ÈýŸÓoÀDFÂß
A1À:N2 ä|À;­.ƒ¡	пۗA¹øx'@š÷0£‹á?û›A9†4¿ïÿ⿹z?ïþÌì­<å¿Ñ	Bsíã¿ÜS.¡UNASNone@¶=ó¶E¢PowerLawnone?ïþŒÑ#¸?`ÏÑÒ¯?'?næló?`ÏÑÒ¯?ïÏ;¢—v?­_1.oV?xb.ÿ3Ç?­_1.oV?ïÜJ?fåÖV‹ïa?qˆ|®®Öü?fåÖV‹ïa?ïøí¦ß'?<GH[ÅÃ?LK…*=5Ï?<GH[ÅÃ?ïþíœƒ·?":NØB³A?'!(wém?":NØB³A?ï4…]ÓE?°—ö:á&?™o_´E—d?°—ö:á&?ï֭ʏA?u<·f?Ab?t©Ú¥¬?u<·f?Ab?ïÇ'H´æ?rc¨ÜÛ >?|l[½ÔØþ?rc¨ÜÛ >AGN3FGL J2354.0+2722@Zär\=îxÀ@ãÈ}²³FÀ:«ks¡RÀ;þ¢$'–H?Á{µÚv@
œ&"iY
@=ÿg©²¿ìs_ôx¿ÔŠÜŽG׿ǭ€'ú•¿é°6¿UNASNone@ŸåÀ4mÅÖPowerLawnone?ïó‹w?VºHêś?YÒåIpÛ?VºHêś?ïÇz@@•z?Œ¹¹Zæ;Å?|BßŘ;#?Œ¹¹Zæ;Å?ï'ç£nã?‰¹Ê‡:Uî?F;ÐED?‰¹Ê‡:Uî?ïÐôVÔx?^Ïú›"w?w…Ôˆµs"?^Ïú›"w?ïâæ9&à?nßVZ÷?moíTÀ@?nßVZ÷?îðI1ÞZ¥?°Î™øÜlŸ? ûlãÒ#®?°Î™øÜlŸ?î'eB¶=?¦–á½†?­‰«ÐRé1?¦–á½†?îá×ÒJ¡J?•ÉzKºWn?¡â'Ü1Ò]?•ÉzKºWnAGN3FGL J2354.4-6612@s}¼¾aÐÀH÷'·þ	À:?ïXzÀ<»Üº€š?؆èrÖÈ_@"Ú§
@€å¿ŒóC¿àSžˆÛ¿âæoÇIfb¿èGÇûèÕ¿æ†P´@~UNASNone@¬c×
=qPowerLawnone?ïö–Ø9§?WDÏñ¥`?RÒPÑ×?WDÏñ¥`?ï¸÷j°"?3¸ù€?Â%Q7È÷?3¸ù€?ïx¶Øø1Þ?"§ZÈ.Ÿ©?é$ßAöC?"§ZÈ.Ÿ©?ï2ðäóÎÞ?zÓhâ‡î?™¡ãdõÀ:?zÓhâ‡î?ï^_ĉÃ?™[Ɨûé?"4Ŷù"?™[Ɨûé?종bCÛ¼?Àe@Ãáä?ºëÔíá""?Àe@Ãáä?ì¥j7úÿ?¯c$ö++?ºÔ¯&@(?¯c$ö++?æÂl,Š2Û?µ†X"!××?Ò{'¦ëšK?µ†X"!××AGN3FGL J2354.8-5245@tº^5?}ÀO#ˆDÀÀ:åw¾}À;¡7qÁ
?ó!–é$e@q"T[!@C}ßÔ¼Z¿è¯S´KæL¿áòUÎÈ¿æQێþØZ¿ïÿóì)$UNASNone@"%¯4Ö¡bPowerLawnone?å{OÓ82?ÑÚv§íÿ?Õ	`Y›ò?ÑÚv§íÿ?èmç'S‡Å?ɔ=0¯l·?ÎHa¶±àì?ɔ=0¯l·?é%¨¹¥±3?°sùþ²n?Ëi]i;6?°sùþ²n?åé},P•ð?­µ±ÎÕÌ·?Ô-§^Ô!?­µ±ÎÕÌ·?áa#‡)ç?ӊ¤ðK^?Ý=ù¸ñ¬3?ӊ¤ðK^?Öϟ©ÂË?ÒvВL$?ä÷0+š?ÒvВL$?ߕPÑ¡Z?¹R¡ý//?à5W—/uÓ?¹R¡ý//?ɶ§ºw=W?³&WZœ?é'Vb0ª?³&WZœMIXED3FGL J2355.4+6939@]"_®¼@Ž@<œaÊö3À9±a8)<9À;)L$›À»?Ëý5U@
Ò	ÿ2O³@[á ŽÂ?Å%£'·Ôî¿éÞm^°Ã
¿ëšMbx4¿ØôMyÁžUNASNone@¿ÞÑ·PowerLawnone?ïùþN$%N?RÚÒÀHf?HÇñµØ?RÚÒÀHf?ï·Ïá:~<?'öìÚ)ã?'µøä?'öìÚ)ã?îõòçqF?"·5S!yÈ? §àÒdҘ?"·5S!yÈ?ï×ÊàʖÎ?_'±#<0?tµÙ+?_'±#<0?ïÃ)Cp>?‡NŽåRÙ?~k^?÷Ìá?‡NŽåRÙ?îKUr—9?´fcœ%Æ?«J¨Þš¥i?´fcœ%Æ?ì—û;~å?­·DdêÞ?»@'^$Ú?­·DdêÞ?íޖÏB{ƒ?¥cG§MP/?±I‡£ñä?¥cG§MP/AGN3FGL J2356.9+6812@]yèPð@'ó!Ë+ãÀ9oÑI3PÀ:ÌÀˆì?ӍŠÛCe¹@âŒQ²z;@
Aߞ`©¿ç÷݆S¿ëš{8Qøh¿çì"2Á¿ä:Ä—UNASNone@‹ºW^ FÇPowerLawnone?ïõ+j‰X%?Zù0¡"*?U©*'åð?Zù0¡"*?ï¯Å¼¦þ¡?J»kúš¨?"æf·?J»kúš¨?#ÚМ?šÙ9ë?¥]À›(I?šÙ9ë?ï©XØÍü?hiYŒ˜'#?…½é¼$?hiYŒ˜'#?ï>2+\‹W?¢.ˆófç?˜9º—Þ1
?¢.ˆófç?펐è-?¹=+™ž½"?³‹Æüז?¹=+™ž½"?ë(tÎçŒÊ?²šÛ£í??Ã^,ÄaÌ×?²šÛ£í??ì>¾_TVø?¦ì:Üaú£?¾

]HA?¦ì:Üaú£AGN3FGL J2358.5+3827@[ëúÁҝÇÀ7BŒG¡AÀ:0/(âwYÀ;¹‰Úõr¿ØŠ$¾@¨ZéZ¢
@Ÿ?Àà?ïӇ¶–¿âØem~¿â"'«ìW'¿ØÐÁ'°ÁUNASNone@¥üðbMÒòPowerLawnone?ïÿl·ŽL4?°"euÈr?iIìx?°"euÈr?ïˌVÂG?Œõ"ÿ÷}˜?z9ÕëÐP?Œõ"ÿ÷}˜?ïâ;ßÝ©G?j3å[E?mÄ ©x?j3å[E?ïýÑې›)?‰²Î£V|?1q"bƕÆ?‰²Î£V|?ïÿZ¥VÕé?‡jeQ?«XQ#ñt?‡jeQ?ï%¿™;.?°'N¨£…?›^	hþT?°'N¨£…?ï·ˑl?€ý;,	sö?~¤Ró??€ý;,	sö?ïî1oþY|?X¤¨·žl?aΐÆo?X¤¨·žlAGN3FGL J2358.6-1809@P¦ ºKÀR¹G"#ÐÀ:SãD8>À;Äꁺ?今ã¦á‰@.ÉA'?ý`ç÷K¿è£p™+pØ¿š¸þ{Õë-¿ÉÁ2\@:¿ââôxQ9GUNASNone@®ªõÜÆ?PowerLawnone?ïÿWYê=\?
žbªs/?ÇE‰P?
žbªs/?ïÇz˜Öß?Ž¦µb­1B?|B³0'?Ž¦µb­1B?ïæ๋ø?^'ªŸÁË?iFDǀ?^'ªŸÁË?ï¯8Hµ•=?fÀ'*@ß?"1íÎ{(å?fÀ'*@ß?ïþwÿ`É?#»Ù³j?(€ýøwK?#»Ù³j?îë^QˆÍˆ?­œR O°?¡JêÜx?­œR O°?ïÉSY‰^?{‰'TWn?{VS2|àî?{‰'TWn?îçÛl³î–?œ­¡î±?¡'I9™Ÿ?œ­¡î±AGN3FGL J0002.6+6218@]SRÁmóù¿£äVAÀ8¸4t{ÒßÀ;¿"å­?ÿ®	&šI@ù8ö–Ÿ¿?÷;Q­Fʕ¿Áôˎ´8V¿àõø8Ðø¿çϟA›£,¿ïÿÐ%­õ­UNASNone@œ'n—PLogParabolanone?s{èZ|5K?"¦vJÚ?ïÙ/'U?"¦vJÚ?§šGG¡±?¿#z²½pÓ?î†^Ë´Á5?¿#z²½pÓ?©g"èÃÝ?Ÿ¶ò²ôæ?îi†ÁG*?Ÿ¶ò²ôæ?«"'#óÒ?Šœ{6²7®?îF͏…s?Šœ{6²7®?p
h^?•hŒm-W?ïß×åjäŒ?•hŒm-W?d«õ=Ž"?©žÍ©ú6~?ïŠmPTE?©žÍ©ú6~?Š–DÚ¸cW?"‰åü±‡p?ìy¡"?"‰åü±‡p?vþӎÁ§?aÛ¸ey?ïÒXõº'?aÛ¸eyPSR3FGL J0008.5+6853@]ÄOÊB®Ñ@Y»j¤¹ˆÀ9u(>«	À;e£Z»Ð?ýí,€çq@s[T9"?÷ðΑÈêÀ¿Äæ}ß+¿äY_쓀j¿î¾£Fõ¿ïÿbá*¼UNASNone@‰¢¿3‡LogParabolanone?pºÏxf´?"Z—~öÑ?ïފa9Î$?"Z—~öÑ?©zÜÈ ö¹?À@Eþš'Ö?îhR3uð"?À@Eþš'Ö?ĕßâˉ?®V eY®Å?êÚºHM?®V eY®Å?£ü³Ðß?‡+ÎÈK:?îÀ4ÎhÙ2?‡+ÎÈK:?€]2¿Q°?ms€=B¥?ï¿Þ‹L`?ms€=B¥?'äDsޅ?ª g,»?ïwhÞ!;?ª g,»?µ¥2¯‹»Ž?¨&œPG?íKYª7ÃÞ?¨&œPG?bŠ<¬ö?St'zŠI?ïíuÃjgA?St'zŠIPSR3FGL J0008.7+6558@]¦s>»ýr@¤á¼©iÀ9šCã…À;,rÉK8?ý—£FÉ@ÏzÒB@pp€p¨µ¿Ù»0(wÿ¿ëÈvaŽÃÛ¿ãôÄN4Q§¿é쌦t¦úUNASNone@Kx"LogParabolanone?ÀÌh_ 26?ŵFoaÄ?ëÌåè7ós?ŵFoaÄ?¯H§Éê¥?À|O¼€ÏH?îuƒS Ö?À|O¼€ÏH?ã0:2Œ‰?´pç«)ÌÉ?ٟ‹ãšæî?´pç«)ÌÉ?Íoó5ŸÓ?¡É[⫐¥?ë¤2˜?¡É[⫐¥?Á*øž"1u?Á	ÓÜi*š?ëµAØ^ó£?Á	ÓÜi*š?"e_¦å$?«Ï"Ì?ïdÕë·?«Ï"Ì?Ý\|
9?»@˪Áh?áQýAùcs?»@˪Áh?˜¯SYG?"^î÷×Ä?ï?Z… –?"^î÷×ÄMIXED3FGL J0039.3+6256@^c {5*"?º$ª.gF‹À9köÔ{À;AŠ[@	.êú	q@;epÈ¿Á'áÙ¬âª?ïý°3Rׂ?yѦ p&ô¿áä³Ä›®¿ïÿü]šK,UNASNone@œ±¸ºÇËLogParabolanone?ÚѶZ¬…?ØÐÝJî?â—$÷R©½?ØÐÝJî?µjàÚ;n?ÁÀ…80'?íR½Öú"?ÁÀ…80'?µAâ֔ð¿?¥Û¯ÕÐi€?íWÃ¥£x?¥Û¯ÕÐi€?Á¬Îä˜à%?ª2™ÓwÍ?ë"ÌFÙÇ÷?ª2™ÓwÍ?Ðk}»ÜSl?×ɂ.Ã?çÊA"ÖJ?×ɂ.Ã?¡•N@¶Æª?´ý¡Uü?îæ«æÕ%?´ý¡Uü?µŠåœˆ~˜?­Õ€Êq§?íN£LSsM?­Õ€Êq§?œ,<~Huß?"E7"¶™?ïžzÁ?"E7"¶™PSR3FGL J0212.1+5320@`ݧæšÔÀ•&Rz XÀ8ÊYž×ÇÀ;/`Ëò¥?ýyšóṙ@‡/Kòò¦?öۘð&n)?Lóp*¿Ùë»{–¤¿å¤þLf`¿í—*;:ØUNASNone@'·KC•LogParabolanone?V)B±&0?jÞr+3'?ïôë_	$í?jÞr+3'?°'L?Àû"˜½js?íü]?ü§?Àû"˜½js?­Ag2T–?¢Ê틟‹?î+îٚ™'?¢Ê틟‹?¿ò}`}ï?˜D¡k%…?ì°SðB?˜D¡k%…?E!v:µ]??JÉð?µ?ïú·¢WŠ??JÉð?µ?"ôÆ@4±4?¬ézÎ?ïXYÎ'•Æ?¬ézÎ?"ÌÛH7<²?{Õ|*"Dm?ï¬Ì'Ñd?{Õ|*"Dm?'>ºˆ¤L?v[›³*‰s?ïv
+ä­?v[›³*‰sPSR3FGL J0223.6+6204@`¯âXOLn?ñצ_z¹ÛÀ7ò˜ëô°AÀ9àá"-nÎ@»Ð¸ê—¹@
ۚ?±Æ·?ùŽùÕÄm-¿ãÿī웿ہU§Éª{¿ç䌳w¸¿ïÿÖܽ}UNASNone@ŸÉ.Hè§LogParabolanone?DC¾¯ô*?abÔÁ!ð®?ïúï;{oý?abÔÁ!ð®?¥êW£à,l?¿€Ü¯ÿó§?î¡Z…Ýz?¿€Ü¯ÿó§?³QnÎèüp?¥UõþGº?í•Ò%ëæ²?¥UõþGº?š?8Ößj÷?€§üœñ?ï.9;F8?€§üœñ?p°žòâŸ?¥c"®
–'?ïßòžÃz?¥c"®
–'?Œë«êg?ªÒÊʋvc?ïŒQP:ç?ªÒÊʋvc?¡ª¤ÿŠV‰?™_Æt£S?îåU°>TW?™_Æt£S?jyµxõ@©?[n6d¤?ïå†JÃß?[n6d¤PSR3FGL J0225.8+6159@`¸åŸ+©Ò?ñîI9.õ·À8\'jPÀ:ç!éB?úÁ.ãÃ3@¿v×LØv?ü9´¡ÝµÓ?ﻼG¬š¿å"à…Cÿ½¿éäñ
¼¿ï|w@9'.UNASNone@œ3ù	k¹ŒLogParabolanone?Œ.Ð1?—ʭ㨆q?ïD¿UH?—ʭ㨆q?µ/¡¿×¶?Àеëðå—?íZÈÜY?Àеëðå—?Êߊ$í±Z?°Â†ßV?éHvē©?°Â†ßV?Ê$:üj}?¥é—>º?évñ\åa?¥é—>º?XpH4?`§ÜªÉÃ\?ïóÀG"z\?`§ÜªÉÃ\?™a½i•`s?¬½¡ž¨?ï4ò|[=?¬½¡ž¨?³Æ,³Êï¾?ª)ãM|<?í‡:i]f¸?ª)ãM|<?¢棞¼T?Œ*xN›C"?îß•\?Œ*xN›C"PSR3FGL J0238.0+5237@a[&ÉÀ¯"á¬WâÀ9.ŸÇ±À;pÌ؋Fð?ø4eø­P[@ËÊÒ÷‰9?ý;3L³Œà¿âo5ãå¿àà¼;bµ5¿ä&â涿ïÿéò§}UNASNone@oç ù	lLogParabolanone?Г6¤½ö+?ÉØò!<ˆ?ç¶d­¡ê?ÉØò!<ˆ?°%WOu·?Á-'ª'b?íûU:‡™?Á-'ª'b?ÞÝ­ùÓ
?³~ñéæì?à')rz?³~ñéæì?À"¦P[(?˜Å¢|«?ëÛký)6?˜Å¢|«?›:^íî|í?¤uÙÙ¢3¡?ï&-ÕDH?¤uÙÙ¢3¡?'å'Z ¥ö?¬ª¶–bT?ïhÓí8¹@?¬ª¶–bT?À<R6ÆY?ªB!é'ç±?ëðërNj?ªB!é'ç±?ˆTk÷{ËH?oÍu‡u8"?OøՃ?oÍu‡u8"PSR3FGL J0312.1-0921@gðwÙUqLÀJ.U⊤3À9ùíÓ­'žÀ;ͤ¦©M?ö2´ [)Ç@åYŒä)‹?ñ7ð<ªÒ?ÚDñ«±þ¿ßb{$¹rÓ¿â±ï¿¿ïÿö‰£q#UNASNone@'ʁ [ÀLogParabolanone?䟏´µÌ"?ՖùÒЃ!?ÖÀà–"g½?ՖùÒЃ!?âq‰¶ˆÎ×?Î"Ï þÂ?Ûì'îbQ?Î"Ï þÂ?à÷u0È?¹ÂÖÝO"€?ßÕøžo?¹ÂÖÝO"€?ß$罶P×?°îÄl¡«ñ?àmŒ!$ו?°îÄl¡«ñ?Ü*IIõíX?ÕÇÿÏiÆS?áêÛ[	T?ÕÇÿÏiÆS?Ð:j»pë?Ï6uW´·?çâÊ¢GŠ{?Ï6uW´·?Ì*;׋['?³üõÝKÒ?èõq
)?³üõÝKÒ?¼¬\G‡1?¥ÕÔY]?ì|ªtw?¥ÕÔY]MIXED3FGL J0318.1+0252@fN>ê šªÀEÑG®záÀ9ãpñãºÀ;îu"çZî?ûô`΢:@TÍ¿»í,?Ñc"šë¿Ï¡CS‰6l¿½F$ð'è¿åðÄ4,¿îz]ûͅUNASNone@—|"µÜÆLogParabolanone?¤øþ'™T?À:3¾°?î°p­/g?À:3¾°?ÒŽdÃ_?Ð!2߃ç?æýz8͞P?Ð!2߃ç?ÃGPÁIÈ?°67¼³8Í?ë.;ëÏ­Ž?°67¼³8Í?ÍÓv).š?²b¡néÜl?è‹"zu´Z?²b¡néÜl?£j⅝m¢?ÂG£oRÀ?îÉQ×|íÖ?ÂG£oRÀ?¾	¥tˆ?Ç®K	$?ì>ËQnÿß?Ç®K	$?±fÔÀŒ!·?§h›ó+ªU?íÓ%h33ù?§h›ó+ªU?ŸIÒïÂb?"˃nö2?ï±hJõ¥?"˃nö2PSR3FGL J0332.4+6110@a¤u£KÜ@'h	ԕÀ9¥¦&oÖRÀ;]Æ!·à¬?ö£câ"@Ñ•aüt@>í8}¿Ñ½±•¨¿ê?ùái"?¿ê"oGØÔ¿ïÿ3HE­ÎUNASNone@ƒxÍÓØLogParabolanone?ãchu	le?Ë\–í†6?Ù9/í'5?Ë\–í†6?ș‹»Ï=Y?ÄØñ±':®?éٝ0ª?ÄØñ±':®?ä¹Kïf?³Ë~þi¦?×àh!Á5?³Ë~þi¦?ÙÊÈ:ÁÈ?¨ã>U§?ãv›âŸ?¨ã>U§?м(ú†?ÇJ-J»åõ?ç¡ëð~'½?ÇJ-J»åõ?¢Uÿ"ê ?°n¶ÈdÄa?îÚ 
ë¿Æ?°n¶ÈdÄa?Ýj"\¡?¶ù•g6Ä-?áJîÑ·ö¯?¶ù•g6Ä-?©¼v`?¶Ro¶½?îd8žN?¶Ro¶½MIXED3FGL J0336.1+7500@`£~=Á@/¼˜¢"ÕÀ9TîDì™À;—éŠrµ?øÀaÖá@,Ó¯*.?øûiÁƒ¿ÓiՒZ9¿Ü0®.ã(•¿ä׆‰ÇiŒ¿ë)'Jê‡UNASNone@e…8ï4×LogParabolanone?¤rU¤J˜B?³gõyí–l?î¸Ú¥ä'Ì?³gõyí–l?·GÖ2-"?ÂÈÖ	Ù¿ò?í9È-?ÂÈÖ	Ù¿ò?ÚùSg0;?·¬ŽÕ '?âƒVLgã?·¬ŽÕ '?Á¢ûW¤¬?š{Ã7%DÙ?ë—A*ÔÙ?š{Ã7%DÙ?o§TIƒ®­?p÷·–ã't?ïàX«ùÔ©?p÷·–ã't?Ÿªž«zR?²xà»#ÿz?ï«
Û%U?²xà»#ÿz?«эؙ?¡Êîeλå?îNÒçK±¸?¡Êîeλå?‡Lv–®Y?lšïý¢ÜO?ï¡ÂÎNà–?lšïý¢ÜOPSR3FGL J0340.4+5302@bXüø
Ã7¿ýí©¼&ŒÀ8ðà9'À;¸h'¹Ñ?üˆY«ìØ@»OÞ9±¨@ÚYO§ˆ¿åÀï7Ë¿îx¿ž)æ¿ïÿ}…^F¿á@ùðÏéëUNASNone@iðrGE8ïLogParabolanone?éZ"Çfm?ËàaK–ΰ?Ëæ—tâfM?ËàaK–ΰ?­¨kB¾øk?À°5$؅?î%yKÆR	?À°5$؅?çEË'þn'?³r œ?Ñti°#²?³r œ?Á'øí"i?©I'$éá‰?ëŸ\Ä·f?©I'$éá‰?àÝ'\ ¶?҅iJ`:A?ÞE±G¾"?҅iJ`:A?'ڜ?«-çûĊs?ï{s÷®<?«-çûĊs?äÚ}Éü°7?·hÒUN›V?ÖKlŸ"?·hÒUN›V?Œ0Ò·›­Þ?'Ã\ðø¤b?ï<´øUù?'Ã\ðø¤bMIXED3FGL J0345.3+3236@d
ʁ˜ñÔÀ1ZbwÄ\¼À9‡G.'º'À;†@@aïß?ùÄ9-D‰@øc^J8?þÑe*|*s¿¸'©öB¨¿éQDɼ*¿êÛåIxøm¿Üš¾ZԍUNASNone@"':)ÇzLogParabolanone?êü"¼Ý/_?Å耔\eS?Äu‹Bƒ?Å耔\eS?ãüôZ/ve?Ñ+"ý"€?ØK¡6?Ñ+"ý"€?éLxꀞ?±€'	ªÛ?ÊÎUÿ™†?±€'	ªÛ?æÊR@"G?°…R'†5?Òk[úÙr?°…R'†5?éo¼˜ÞD?ÈÙçIr1B?ÊCå
œ†ð?ÈÙçIr1B?ÄN'2[?Ç`x—øQ?êìx_si??Ç`x—øQ?è^Á…,5y?µ¤´@­Ó?΄ùëO*?µ¤´@­Ó?Î0'vLɘ?¿ÜèI')Å?èsö"l͚?¿ÜèI')ÅMIXED3FGL J0359.5+5413@bˆLYtæ\?ëæðY|sÀ8nÌ¡-â'À:÷c°©€—?ý3ù;듌@Ÿô§‡C?ük—›<±â¿Öa78·"¿âi‰Ë45+¿æ7ÛÓ>Æ¿ïÿç—åu¡UNASNone@ˆ!BpLogParabolanone?"LbSæi?ŸÙý)9så?ï®Ïª]ó6?ŸÙý)9så?¦.ؒu/y?À+lªÎ]?îv"ôÙ?À+lªÎ]?ûñn O?¯'ÄE7ï:?ë>¤Wì?¯'ÄE7ï:?›Æ5àµØ'?{^;9/?ï!ÎQ1Jü?{^;9/?tõÃϗ¿9?¥,ŸÉž?ïÖxvÎ?¥,ŸÉž?Œg)g©ó´?ªÛa?T—?ïŽcZ˜Qñ?ªÛa?T—?—H¢væ?'V9ÒÇ~'?ïEºëŠ
q?'V9ÒÇ~'?a2JU½ºt?K«¯Ñ¥Z?ïî͵wh?K«¯Ñ¥ZPSR3FGL J0426.7+5437@bÛ¾ ºK@ý¸ýâïNÀ8'£A¹ôÀ:¤UÖÌ*@PŠÇn¾ú@•†ø,L?ýæðõvO¿ÌÖùͶ¿ãUº¿ìÝõ›W_¿ïÿDUNASNone@Š Â\(öLogParabolanone?…§¬›˜¼?'ÞۃyÄ?ï©aMLäà?'ÞۃyÄ?¨ôjüqVå?À+Þ¾oo'?îp¹P¯B?À+Þ¾oo'?·¦¡±¬e?¦D×k#sÿ?í+É¡8
?¦D×k#sÿ?®.ÌrêN?Ñ‰Wԓ›?î8ìۋ?Ñ‰Wԓ›?ƒ^—jd?©ãϹ4k?ïÀùCð'?©ãϹ4k??ÒYÒÏÞ?ªç%)>Å?ï~mhcA?ªç%)>Å?–æŒۑ1?"Œs累¨?ïH˟¿è'?"Œs累¨?yX¢X"üT?f'§ìƒ;?ïÍN»,™ð?f'§ìƒ;PSR3FGL J0431.7+3503@d·BZîc À!Ûà›¶ªLÀ9Aû§««À;"n@O{?ö>?Þ½:3@cŸa¯@¿ó£%^‰¿æcb	¬Éo¿éIjX×v¿ãH VÑaÌ¿ïÿÃλ(NUNASNone@h€hۋ¬LogParabolanone?ì+çY…?Àc*ò>n?¾ Çm3×j?Àc*ò>n?ÎRÜ'1ã?ǛW\»ËP?èkHúßs‡?ǛW\»ËP?èßÜs€L¹?¯;Tˆ&µ?̀Ž1þÍ?¯;Tˆ&µ?ÝØû)ªJ?©»¾þ"?á'kªÛ?©»¾þ"?ãFQ@—þB?ÑÜdokH?Ùs]~Ð}?ÑÜdokH?§½µ›—p?´ªA?Ïô?î"$¦8ʈ?´ªA?Ïô?߂"ó'³?¶nÎÿ¿ÙÃ?à>î†l&€?¶nÎÿ¿ÙÃ?¹
[š©'? •x°g|Á?ìÞ_"äŽ? •x°g|ÁMIXED3FGL J0514.6-4406@o/-w1ÅÀA²DêÀ:å	ÚtUÀ;Õâ˜,ž?öýOòÁ`@K&Ðú.@œ¹a`B¿Øda~u%ò¿æñye­¿ý¿ïÿäÙ«Nð?ïÅ7ƒ5:[UNASNone@€¬±&éxÕLogParabolanone?ïskºÀ{?žÌ³ft?''ˆº@†˜?žÌ³ft?ï»]i›,Ê?"±ñ«Þ¨ˆ?(¥Œ~??"±ñ«Þ¨ˆ?ír$=T¨?¢§Úõ»u»?³"nÝ9sÃ?¢§Úõ»u»?ïî·l­=?bï-"¦x?aH"0S^?bï-"¦x?ïZìñ8ª?£>"
Iµ?"¢aÐeļ?£>"
Iµ?í'ìÖFb? –BÍ*?³op˜ßÙq? –BÍ*?ëA–~9ÊZ?­–18¿á˜?Âù¦֙?­–18¿á˜?î©AÏÙ?³nHÂÛj?¥nKær
@?³nHÂÛjAGN3FGL J0537.0+0957@hiŠ	ÞÀ'(÷À9˜K»ÀÀ;2(@éÈ?÷¸ß9áÎ@ÒåE°a@M:*ž9<¿àNéÐÒk¿ên¹ª¿ì\kñô,@¿ïï–û¦÷HUNASNone@z2±Ä2ÊXLogParabolanone?ïÞ´Ol=°?£ ýø$$´?p¥ØBR7?£ ýø$$´?ï:ÓkÁç?Ÿµî^Îߥ?˜¥Ÿm`Y?Ÿµî^Îߥ?î ´â0h?–"ǿ"<?¥ô±Þ­÷?–"ǿ"<?î3Ö䨶˜?‰7Ìòrµ?¬Â'³¼È'?‰7Ìòrµ?ïë]	š0?dôwµ;<?d¢ö^Éh"?dôwµ;<?ê£I?Rêø?Ãè•òt*?ÅrÛ´T?Ãè•òt*?íÃÙÌÃO?¢'οºAd?±á1šU!?¢'οºAd?é"Ž	–'?²¼;NŒ¥?ËuǗ٥ù?²¼;NŒ¥AGN3FGL J0539.2-0536@j5®h]·kÀ2›bÇut÷À9@[9âyÝÀ;3whí)d?úAN*…@WMç'@oñ§ÍŽê¿ÄеuÔS»¿ìÝÔ'¿çžr'—ír¿ì'äuNÐaUNASNone@ažì¿±[LogParabolanone?©ù Ý‰D?µb=Ž=?î`eò^gû?µb=Ž=?³…aE˜¥?ÂóÖµó†9?íŸ/S»Ð?ÂóÖµó†9?ßó ßì?³@§/ÇRk?àwòï
?³@§/ÇRk?¸xþ䢛?–¯p½?ìðà#'½?–¯p½?šßö§º?©`ä集ü?ï)J¹ÈÊ?©`ä集ü?›Ê"P÷d1?³=m\\Ÿ?ï!®íO	?³=m\\Ÿ?Ú³²n¡?·ÀëȜƒ²?â¦&Èõ/u?·ÀëȜƒ²?9]oü?nõR侯ø?ﻃÉ|X?nõR侯øPSR3FGL J0541.1+3553@e²PÅë1<@¼÷S½À8¹ÈÓC"À:É(çÖz?üӮɺe@{%Y*éŽ?þáñ¿Ò̒…(Ht¿äh³Î¶W¿é¦Îb›x
¿ïÿÃÖȽãUNASNone@'z]æšÔ,LogParabolanone?·'4gqå?½NZ?í}÷Éó?½NZ?§±SÎu?À0Èl7X(?îŽt︁‰?À0Èl7X(?ϟ@º&ÏD?²àÅsA_)?è/ÑvL/?²àÅsA_)?¨
Éò!Ò?…&74:=j?îŸSSs?…&74:=j?ŽCÇQ¤·?«À¤,gš?ï†ð⫱I?«À¤,gš?`þ¾#¡!?ªÙaù¢ÌQ?ïŠ|Þ6,?ªÙaù¢ÌQ? ÷³'a?—±mp§Ð?î÷ "ž¤Š?—±mp§Ð?mѪs°Í¥?W‹kÁx?ïâ.UJV³?W‹kÁxPSR3FGL J0545.6+6019@câXOLn@/©Á/	ÙÀ9'jËΠÀ;®.Me?øKÂ@¨^ùŠšù?ïdã&€rV?ۇŒ»ÿd¿ÓÂÊ$ú¿ÙWÍW\¿éƒ'ÆSÈUNASNone@ä>ߤ?æLogParabolanone?×ud§Z³'?Ï­ÉÔtâ?äEM¬R¦8?Ï­ÉÔtâ?Ěu.!ÈÊ?ĸ†¤ti	?êÙb´wÍ?ĸ†¤ti	?â‹Z›?¸S'y>Û2?ÛòéKÞzÊ?¸S'y>Û2?Òî6'%½2?©è¾µe†?æˆä¾í!g?©è¾µe†?´Ô4Wòñ?º;…
Õ¤?íeyu°?º;…
Õ¤?«9¶û—J?·M7ПW?îLd+?·M7ПW?É,vBHò/?ÀW³¬P'¤?é´âomÃt?ÀW³¬P'¤?ª¿cõÌ4?'Ùä	þ|?îT	ÀÚ6~?'Ùä	þ|MIXED3FGL J0634.1+0424@iáXâe¿ýRøBÀ7Ȗ'•¿À:'zÁg>@Î郑Åe@¿Ê˜@"—hk¿ÓÎÿ‰"ðâ¿è"Dtñf¿ë0yTª§3¿ël›ÿÐZKUNASNone@nýŸÓo~LogParabolanone?'¯úûÿ€V?"y>7Õ!?ïµ@SZV?"y>7Õ!?£ä^9ÌH{?¿íÇÝénˆ?îÁºpùè?¿íÇÝénˆ?Ϻ@7þt?²'ïí•?èoòbü?²'ïí•?…:›!þ[?kkȑX÷K?ï«"¡CB?kkȑX÷K?W£U0À?Œ‡&'ÿ+ø?ﺡt‡õ?Œ‡&'ÿ+ø?Š"EF?ªÚO´%%?Éá,x?ªÚO´%%?ÇßÛ_=?³²ÆG×Âæ?ê	(?0º?³²ÆG×Âæ?O×ÿì‡]1?BoÇù˜¿?ïø
¦N?BoÇù˜¿PSR3FGL J0637.5+0418@ið9–ú'è¿ñßX{ÆJÀ8ÅÞSÝͦÀ:¼hA1ùw?ú¶dÙ"@@p"Í@zlnh¿Âۃ«¾οêCnJœ—Œ¿èÌ׫ðV¿ëÚõªµ/UNASNone@Š"HŸ@¢‡LogParabolanone?å
ëÐëaÛ?ÏNHʦ?Õê(^)<K?ÏNHʦ?Ԙó.¾âÝ?Êì@c%?峆h Ž'?Êì@c%?ä¯lŸæ?³ûH>	?Ö¡'ÀÁÚ3?³ûH>	?ᶠ¡0ù?©›ëùû¿?ܓ̾½ž?©›ëùû¿?бöa¬Ô?ËxÌD'ª?ç§r"Ï)–?ËxÌD'ª?­7V'-Ñ?´3œìì?î/ìŠ_óc?´3œìì?ÜRo·P—P?ºœ‡Ó§,?áÖÈ$W´X?ºœ‡Ó§,?ÄÒÞ¡WöY?¨Ÿ_'ü²?êËHWªj?¨Ÿ_'ü²MIXED3FGL J0641.1+1004@iY;%oü@õ¡lèÀ8·àªÐ"ÃÀ:¾­'tâ*?øz0gQ@†IŸ0\i@ªñó—¿âE":{•¼¿çOx1P@E¿ï¹8Î?Ð W3¯tUNASNone@€ògƒùLogParabolanone?êlRšgÛî?Dzñw"¤s?ÆNµ–`J?Dzñw"¤s?ꙃÔáCQ?Î݃~,p?řð¬zòº?Î݃~,p?ëIÙ
s?¬=!5¿0€?Â؛—ËŽ3?¬=!5¿0€?í"Íîq‹?§øX3Ö¬?³ÙŽœÕ'?§øX3Ö¬?áþÓsŸ?Ò%j6™]ù?ÜÊYäÂ?Ò%j6™]ù?ÓÜhX%}_?Ó#ëJCùˆ?æËÓíAP?Ó#ëJCùˆ?æuž¿ëŠ?´WÈ%Â3?ÓÖ€(ë?´WÈ%Â3?á&šºg*Ã?КÓæqŽŽ?ݲʋ1ª{?КÓæqŽŽMIXED3FGL J0704.1-1043@kýHýŸÓoÀ¯"¼
êÀ8ƲœŸÞWÀ:W™?÷Omü]@
µEw•Ü@@-Ëë%¿á¨|&Ö¿èû0•ý‹d¿æì.wпëAßQsUNASNone@­'ˆÎp;LogParabolanone?Ü?E³œÜ?ËZã'צ?áà]&1ÿ?ËZã'צ?¿ŒÐªÊ:ï?Â1°Ò?ìeꦸ¢?Â1°Ò?ç"4N€Œ?±îŒî™?Ð÷—bÿöè?±îŒî™?֕ )šqõ?¥\Ï."÷?äµ/ë2Ç?¥\Ï."÷?²8Ÿp،?´¢ew×fª?í¸ì­ô½?´¢ew×fª?• ìñ›¾V?­ö_€Â?ïRø˜W¥-?­ö_€Â?ÔÌ=¹Q£i?·°jÒ*—?å™á#W.K?·°jÒ*—?¨L)ª"?Ž#œ¹Êì—?î{>=Ž'?Ž#œ¹Êì—MIXED3FGL J0711.1-1037@làuöý"¿à"5Iè‹À8õLÓi©À:˼zo1ç?ø—h\4ß0@
?Qkr•@¼1ÊèF¿â{ý3¿åÀ´¼Œ¿ì?_®]ÃL¿ïÿh¶«UâUNASNone@ŒßØy=ÙLogParabolanone?Á¤œÜ3	?ÁŸ…÷{L'?ë–ØÈó=>?ÁŸ…÷{L'?­£wö©Ÿ?À)éžOó?î%ȀP·?À)éžOó?á¾öÍs³"?³Éh¦Hí?܂e™»?³Éh¦Hí?Ãj^Ûq?œ.˜wcAv?ë%hxÿ	$?œ.˜wcAv?…g©—?•™€¨ç?ïªý™&
?•™€¨ç?Ž~£ñw¬(?«Â"X5?ï†p,bß?«Â"X5?Ç©õ(ØÞ ?°VŒû6Ó¸?ê'µÉÈX?°VŒû6Ó¸?‡º¤]ê?sVîñ‡9?ï¡oº`?sVîñ‡9MIXED3FGL J0737.2-3233@nÚðEwÙUÀ",Ë:%–À9iÃ9À;6~=ó€–?üÆ~a"Õ<@¶ë+g?üòok²Ù¿ÖQ'[0õŽ¿ä½óñ‡¿ê½?á{¿ïÿÆM¸UNASNone@‡cQ·XâLogParabolanone?Ь¯!&|}?ÊÚë¨Hù?穨olÁÂ?ÊÚë¨Hù?ªí_ʃ?¿ÊÑÊãh›?îQ*P?¿ÊÑÊãh›?ԗ *öVg?µ…<ûè?å´oê"ÔÍ?µ…<ûè?½û†ÆÁ?—%,0fx?ì@>nG(?—%,0fx?—²d'3?¤'ÿ¯IÅv?ïBlÞÇîc?¤'ÿ¯IÅv?ŽÇÎj™—d?«œÐÛ¥-?ï"àÆ:Ã?«œÐÛ¥-?¬îà¹aâ¨?¤üËù&î?î1ô…^µ?¤üËù&î?‡HYµþÕ?r5¾;"!x?ï£öÞToÕ?r5¾;"!xPSR3FGL J0744.1-2523@n*Ûa»û¿æ\°ožôLÀ8u~ÚÑrNÀ;
üaåÎ&?ý
ƒqd]@w@Úæ•÷?ÿ ÛÍp¶¡¿Ú&枰¿å¾3Cû¶¿åþs0Z¿ï‹žw"¤UNASNone@"H˒:LogParabolanone?½{
"µ©<?Ån5óVú8?ìPž¯iJØ?Ån5óVú8?«º7(H9?¿­2#yèà?îN4\d@-?¿­2#yèà?ݑFw]°?¶£"æ0¿ô?á71\ÄQ(?¶£"æ0¿ô?Â؀	O´ô?šlIj²Dn?ëIßý¬Ã?šlIj²Dn?Œ8+Œîü?'ó…ë‰Gß?ïQÌGä?'ó…ë‰Gß?íF9×.?ªêö҆s?J°ä?ªêö҆s?É<LIã+'?¶OÒyÂS?é°ìí‡5?¶OÒyÂS?"MP5"b?|×_Ԑ%?ï]•~EÄõ?|×_Ԑ%PSR3FGL J0758.6-1451@m>·€4mÆ@?W´ûßÀ9¤¤ü¤*íÀ;"¥]òú?÷3*#êì@
;T˜Þˆ·?÷©æU´èU¿ÑËÁÀÔǿ҄‹rù6¿éªí_Gò¿é¿jœw^UNASNone@`}¿H€LogParabolanone?˃ò팤­?ÈÖËÅåt?éDœÖÕ?ÈÖËÅåt?À§¡¼0{?ÂX5|ŸÉñ?ëÖ<óá?ÂX5|ŸÉñ?ä1…à÷?·
¤øt$Ó?םõÚô>?·
¤øt$Ó?ÓÃaœ±?§6úJÛܺ?æ}~O1¨?§6úJÛܺ?•]G(¿"?¡ÕÙ÷éÂ7?ïUƐȐ?¡ÕÙ÷éÂ7?™mI€0û?¬Ѿ>¸¤?ï4—uÁ¼è?¬Ѿ>¸¤?óõ_)?»iý¹mŽ=?ë¨?¾v?»iý¹mŽ=?œ&l¼›ñ?…ÛëÁµ–?ï̙ÿ£—?…ÛëÁµ–MIXED3FGL J0839.6-4133@pRJB®Ñ9?Ô"}Œ.À8†à"&þÀ:šˆŽ¯ZÌ?ýU9Ý@ÜzÛéJ\@™V¸É_°¿hZÀ
¿íø[ª£é¿ëYb…U?¿ïþ/¨0­"UNASNone@'^J82LogParabolanone?1f¥1š…?¤…uP]<P?ïƒ:e4?Ö?¤…uP]<P?¦¡ãÒé?¡?¿À%I—½?î•áÂìèæ?¿À%I—½?Õ:Äg?³I.^ßR?åbüL9?³I.^ßR?·xiSÛ¾:?•ú§œ(ω?íòÕ[Lé?•ú§œ(ω?"F¥''«
?•º‡4n?ï®åkT6ä?•º‡4n?‹Ôwr¦Y?ªúċB_?"Ÿ§?ªúċB_?ÐP^½$¹?·¬Ãl?çõWСm£?·¬Ãl?ƒØ úÒé?q´*˜Lç?ﰟ{õˆ?q´*˜LçPSR3FGL J0847.4-4327@pxdZ¬¿—»»`|;À8DmØJ¯À:f]@L÷*?þ(˜¨-G@îþ—@ã?þÁyŽ°\¿´Nµ—<wI¿èg×Û|E©¿ï9EÍÙV?ÁY­Ñ	‰UNASNone@Š‹åÞÊmLogParabolanone?ĺ‡XÿÓ?ÆNì"Ñ«?êÑ^)߀?ÆNì"Ñ«?à-çˀÇ?ÖÙïÅ9?ߥô0hþq?ÖÙïÅ9?ààϱÁÑ?½åömÉËÕ?Þ>`ú|]?½åömÉËÕ?çÇX`¶›?¼)_¨dÁ?ÐqO>'É?¼)_¨dÁ?Ù(ÎÈPU?Õ»^C	ó?ãk˜þ×Õ?Õ»^C	ó?·Bž‡=l4?ÅÕÙÀ…?í¬/&é?ÅÕÙÀ…?àÉäúYç—?»óçÖ_ë?Þl6L0Ò?»óçÖ_ë?Ó0ðºà´?ͤŸ§Oº¨?æg‡¢ü&?ͤŸ§Oº¨MIXED3FGL J0851.4-4244@pvü;Oag?ïÇõݒAáÀ8UÛ¢R¥¿À:iΐò++?õ¿§@f"@
ð¦z'¹W@€'µ¦•¿àÉIY²›@¿ê¶år
3‹¿êØ[#*¿ã{Ìй҅UNASNone@…%•a'LogParabolanone?âÚÆ –kš?ÎÑëqÊêí?ÚJr¾Ó(Ë?ÎÑëqÊêí?ÒH×µ3(!?Ì'Ôôþ?æ۔%fkð?Ì'Ôôþ?æY0¸¯‰p?µ
h•"ñ&?ÓMžŽ í ?µ
h•"ñ&?áÄÜûó×?¯ƒ(Ô_"9?ÜvGÀR?¯ƒ(Ô_"9?Ç=ï.¡~?Ç_¸ç™r?ê0"4W {?Ç_¸ç™r? g%"(?²'cœ•I?îù§•R/?²'cœ•I?ÞOõW̬?»›ØÅö¼,?àØTuª?»›ØÅö¼,?¹Í¨nÀt?«3þÚó?ìÆJþ''ñ?«3þÚóMIXED3FGL J0854.8-4503@p™¤ü¤*í¿—tR§¬¬À856£*<À:ŠX;*xz?ýã!°SðB@qíVD?ù-Ö|ùÑ?Ó¬¨Üì!¿Ûɽ£º¿æ4È«ø8¿êc?Dä`'UNASNone@›ê5Y³Ð}LogParabolanone?yùÃÜ?™E'Çlƒ?ïÌyú±¦?™E'Çlƒ?§DJ1g/?¿qBn=?^+?¿qBn=?Ê?YZU?³!ُ@	?ép)©z?ë?³!ُ@	?¹–¹·¾•?•_D#¿z?ìÍ(É-\?•_D#¿z?XÀ'È•=¾?ZáNׄð?ï󟶂ø1?ZáNׄð?Œ¦
(.2È?ªí8ññÆî?ïgËQˆÅ?ªí8ññÆî?'qüäÅüt?'ê3±i8?ïlpõLü?'ê3±i8?Šà9ˆ
µ?tÔB‡ÅùÍ?ï"}Êþbé?tÔB‡ÅùÍPSR3FGL J0855.4-4818@pÂq!«KsÀcҢϣAÀ8gQÌ{n5À:vh@Žf?ÿ‡	½=ä@,/±™Ä@7ÒT¿×H1Ð¥¿êtþÙ»7¿è0 ûHòH¿í¨šêbÆUNASNone@‰r¨¡ß¹9LogParabolanone?U™¸Ñ¬ÖC?dgÍ^å?ïõ3#Ս?dgÍ^å?£¸+{ºÔ?¿–Ç"c0?îÄ~Í:…ã?¿–Ç"c0?ѸC¡HO?²º4oæp?ç#Þ/[ôY?²º4oæp?¡4¡ˆ«?'Ÿ4/¨?î°{ˆ?'Ÿ4/¨?x×5Ž[½¶?…'ÆÅ
†x?ïÎQ•& Ü?…'ÆÅ
†x?‰¶í÷ƞÖ?ªñ÷x£Óû?ï™$G÷ª5?ªñ÷x£Óû?ÍÍÑàîþâ?·e£™ˆãÐ?茋‡Ä@G?·e£™ˆãÐ?iÄ#[Pë?Y« li…4?ïæç;ý ï?Y« li…4PSR3FGL J0857.6-4258@p…"ÿCAž?ûP¨È%žÀ8yÊU#HÀ:~ϟåãõ?ø"Íû U@k€´›R¬@ä€ðÖAk?¡
Â0h¿æwúٚn¿ëJ¹4-¿ì'ïHͤ8UNASNone@'Ä6"Fs'LogParabolanone?Ðü«SÍ©ä?ÈÚ¶ö²ày?灪V+?ÈÚ¶ö²ày?Ê÷{4‡NÇ?ßþBe«+?éB!2Þ,N?ßþBe«+?ßÍxƒÊOo?¶~ß«?àC¾ØI?¶~ß«?Þ(N¾)?¨'c{¬?àëØ ër?¨'c{¬?¦ÚÒ¤÷Œ?«rƒÎRÊ,?î'RՇRç?«rƒÎRÊ,? OD6ÀÐM?®YuŒNK?îû¼¡±k?®YuŒNK?ÈéY·ù£g?¶˜ÇAtI?éÅ©'—&?¶˜ÇAtI?·Ýv…p×S?žs¿Î°©?íQ/6h6?žs¿Î°©PSR3FGL J0858.6-4357@p";dZ¬?óN~é+0À8;IàâÀ:o²'ž«Q@Ïh5ã@(ب"H?ý$…(0K¿ÐZ"¿æÆĤNT¿îˆ
Aпà.Ý
6ÊBUNASNone@‹Ë¦ YŸLogParabolanone?Í>MB¨ò?ʹb&ñ†?è¾0l¯UÄ?ʹb&ñ†?µ"—[Ž¸?Áߗ¬ÑÒ?í\-mK‡é?Áߗ¬ÑÒ?à'0Í/ü¦?½ 	þº
`?Þ۞e µ?½ 	þº
`?Í*˜*ób?°&nsˆà?èµxÙõC'?°&nsˆà?Ùf{ñ#T?Ô?…UX»È?ãLÂnUÀ?Ô?…UX»È?'{)ƨ?¬N²·ðE?ït'ÞÛ?¬N²·ðE?áDÿl˜j×?»µ`ls"?Ýv&Ï*S?»µ`ls"?¢×"lÓì:?¢9,<6!?î҇¹iºü?¢9,<6!MIXED3FGL J0901.6-4700@p½o?Rü&¿Ù@ÝÀ»À8 Eð¥À:OY•?úónçê4'@	Wze¤?ýckw¶¿ä3ˆ"¸$ä¿âš¨Éüý†¿èá›Õ¿ïÿ²§ "ŸUNASNone@"äöâëCLogParabolanone?²Ý7z=ÿW?¹µ-–2©B?í¤YÅþ…?¹µ-–2©B?º>ý+d\Ì?Á3.'¹5?ì¸ Z"tg?Á3.'¹5?Ðß0^Žøù?³`G€›?çgиƒƒ?³`G€›?Óu32ÝM?ª«¡úað?æxEff'Z?ª«¡úað?z«êÿè­ÿ?¥éù™¹™?ïʨ*.¤?¥éù™¹™?"èjC2N?­•¼@(2?ï`¼­½4v?­•¼@(2?©Ñé'? MB¹D!?îbïÎÚn ? MB¹D!?¨YY†°¾?•…xÒ*r?îzjg°pÿ?•…xÒ*rPSR3FGL J0905.6-4917@pà
å6P¿öÀ³Nv…˜À8†î‰µöÇÀ:¸šs´-@"
¼õ@X‹{ô˜?û?‡ñ\?îê0õ/0^¿é=KR8Üë¿í<Ž"ER"¿ïþvì#1çUNASNone@ˆÆ?LogParabolanone?˜ÓYÍI÷?¡,ymYi?ï9côú›ñ?¡,ymYi?¤‡»Õ±?¿‰])"f_?B¼µu?¿‰])"f_?ÒÐØþ'ôg?µ	"^i=?旓€·Ì?µ	"^i=?§¸U†7¸?Žá"–ôn?î"z§Õ¶D?Žá"–ôn?£—®±#'?¬ST^"¶h?îÆö…>)?¬ST^"¶h?‹ù"'°5?ªñãD£í?ÎÞ?ªñãD£í?Ñ
À[Wó?·蘳ª7?çzŸÒTy?·蘳ª7?ya#DÌbm?lÞ"°
4U?ïÍ=¹° «?lÞ"°
4UPSR3FGL J0906.0-4705@pƖOv`?¸–º›¡À8²äǕUgÀ:}‹–¡—•?ù"Ÿ48@ä@,9—ÑB}?þÆÌÐ}±\?˳–áÈ ¿ê0";¥Œ[¿îøì»Þ±?§gji͛vUNASNone@‹x7´¢4LogParabolanone?æ½:¸±?ÐóítÁ?҅‹ðŽè?ÐóítÁ?뵯™'"è?ËC'%H—?Á)A™õ¬a?ËC'%H—?ça±)…Õ?³äÊüGw?Ñ<­ØôV?³äÊüGw?íñïÆ÷Ë©?¡ó¤kÉkˆ?°pÉùpµ?¡ó¤kÉkˆ?â[ã¶HPý?Ô
–¯·ñ§?ÛH8"o^?Ô
–¯·ñ§?×Z9$A†?҆èÏ.H_?äRñãmß=?҆èÏ.H_?äòXÁ}P?·ý'™y‰?ÖN}Åa?·ý'™y‰?äJX`5Â?Í{Ì:fê?×ÉkO?"|?Í{Ì:fêMIXED3FGL J0907.0-4802@pӓ ٔ[¿Ú¥¬ÍSŠÀ8Ü滋[éÀ:›#ôÑΔ?úßÐVD/@
©¿³´£?ù2aŸb?ïÿ9†$¿ç×e¿èšg!¢<*¿ïÿ¢å8¿UNASNone@•smw1ÅLogParabolanone?«ǤCì"?ÆE]	ù܃?ëUïÛ?ÆE]	ù܃?ªï9Sö±ª?¿r™
䛲?îQj¥?¿r™
䛲?ռ˰˗÷?²«ÃKpv?å!š'š4?²«ÃKpv?ÁïþD5?¡3£cH¯?ë"<Àz®ó?¡3£cH¯?¤âú.Ük¹?¶â䕅&µ?î±Ð]-¶$?¶â䕅&µ?ŽäàcdÌ?ªýc*@r?ï"l~Xu?ªýc*@r?ËTjK´p?´z.±x›c?é8*åmä?´z.±x›c?'0_ï(í4?€ICO?ïn}†¸–?€ICOPSR3FGL J0914.5-4736@pÜk;¸<ó?飺º{'qÀ8/·}°/À:žQY•@!!Ðà,Ñ@="àø(@÷(pa'ë¿ÓÜR>™ÌM¿ê"åʬa¿í(åÂŕ¿Ò?ÏezÐxUNASNone@ƒT¸ºÇËLogParabolanone?Ý«–'Jq?ÐÆmü¶?á*4¶¸ZÇ?ÐÆmü¶?Ón»¼{"A?ÑâUB°1i?æH¢!Â6`?ÑâUB°1i?äA9
ñ8?¸(¤Æûà?×Ý}ä?¸(¤Æûà?âRý"`Þx?¹r]E?ÛZ÷>C?¹r]E?á'M§þŒ8?Ð&Þn¾WG?Üûd°ç'?Ð&Þn¾WG?¨4çà›Ù?ºxdw›9y?î~¬±öB?ºxdw›9y?å<ð•©?¶àdÚEÀ?ՆõúÔ®?¶àdÚEÀ?Ç¢ÑUŽî?Á1íœê˪?êKª½D?Á1íœê˪MIXED3FGL J0915.8-5110@qÚ{9¿øMzÂ=ý'À8ÞfRDpÀ:ÏÍ"]"?ú•M8`D@õš9ý|Ã@a®‹™%Ö¿ÜzS®'ñ¿í ÙoP"‹¿êOÅóiĕ¿ÎõJ¤mªUNASNone@vTA5TvLogParabolanone	?çþÜÒ(S?ËßfžUÒ+?ÐF[®ýY?ËßfžUÒ+?Ò®ßrR.?ÒÏbS\I?樐FÖöi?ÒÏbS\I?é=ªɏV?°þ9DÆã½?Ë	WŒÙª?°þ9DÆã½?ä\^L';?¹Èï)i'?×GCÿfۊ?¹Èï)i'?ÛQðÃL?Ð
Y·MÖð?âWwžYó?Ð
Y·MÖð?©h®%}ú?¾"þ!zñ?îiu¨ _?¾"þ!zñ?åg‡1ÑÎ?µù4sâìB?Õ0ñœ\cû?µù4sâìB?Ë
{¯Š?¿L·†P?é<¡~?¿L·†PMIXED3FGL J0933.9-6232@q£Âã>ÿÀ"`úÛÀ9¾ÙÅÔÀ;" ¨ìó´@jl(T@RãKζ¿×ÎR8œ¿Õ™éº]"_?°ïÒq¿á¤"gÑK¿îÊW…*ªVUNASNone@šÄ7éùrLogParabolanone?¿úH
¾b.?ɚ`E:?ì¶þH3º?ɚ`E:?®bWéïôú?Àk\fՙ?îځ7Åa?Àk\fՙ?±¶ò_¢_¸?£I:œäÕ?íÉ!´'0é?£I:œäÕ?³¼"$d­7?¢ÞP†>î´?íˆm›J/	?¢ÞP†>î´?ÃfQ°ö?ÓÙò÷Ñ)Ë?ë&xk»SÂ?ÓÙò÷Ñ)Ë?'™._šâr?¬d‹Ó"ã.?ïs6¥Ì?¬d‹Ó"ã.?®B1û^»?ª«­S[ö?îÜï§Å?ª«­S[ö?…)	鬺/?"z~©"Å`?ï«[ؐF×?"z~©"Å`PSR3FGL J0953.7-1510@o~"t¼@=šÿ}úâÀ9Ý8§z¢À;ùõ3c¾?üR:Ð5@
É))D?Û«g𲸭?èz;ì{z¿ÎOo -¿çnS	½C¿ïÿ¬r†§œUNASNone@•á–R½<LogParabolanone?'ÍmEMž?šÅK@±?ï´ÊJø‡ø?šÅK@±?º:ߏ?ÄfӓæQX?ì¿X½ÜD?ÄfӓæQX?Á¦§çÎu?®Ëy?ë–V†c?®Ëy?³
%·D†_?š¯à¥>5?íž[I@ª"?š¯à¥>5?†èÍ "&?•êý j?ï¤\ËTt?•êý j?¥ö'W—?¸}צðo>?î® «f?¸}צðo>?ªêoÁSÔ?¡-övSY?îQ^:ä'?¡-övSY?wA\¸²úl?mA¹hØåÂ?ïÑ}FZ_û?mA¹hØåÂPSR3FGL J0954.8-3948@p݂ýuâ@&ê@1HwhÀ8¹}uv¤¢À;m2˜Ù€9?õËÔ.ÀÝ«@×-xß@a9n'Z¿ãÒ¼"Ëÿ¿èŸ"L±¡¿ä‹»S8óM¿ïÿ¢Gƛ¹UNASNone@uÁ
Ã7!ÕLogParabolanone?ç¸åöÙ)–?ÉԇZ–"D?Ў4M¬Ó?ÉԇZ–"D?¼œõ5ª:?ÿ™H?ìlYJ¹?ÿ™H?é`VåÈyß?®Tá3Û%Š?Ê~¤hÞ'?®Tá3Û%Š?ѹ$B™F|?¥F}òÚ¿?ç#mÞ³\Â?¥F}òÚ¿?Ö¯Ž'öi(?σñžŠ¼~?ä¨8ìËl?σñžŠ¼~?ŸJ7Vv?°S'N¾ÌP?ï®E"I?°S'N¾ÌP?Ý9Ò§µÄ¦?¸·¸Š¶??ác¬%­?¸·¸Š¶?? p5ׄ4"?…o
T
Ñè?îøü¢l?Þ?…o
T
ÑèMIXED3FGL J1002.5-5709@q˜îcŠ	¿÷ƒÆÉ}À8kõœÏ®ÿÀ:O#
KB?öæä‹/s‹@œJ‹¿f]@Â@VÝ1?ÕÆ•^ ¿è	·}œ¿ê1øJ©òW¿êj_«rpUNASNone@ŒxkP°ò|LogParabolanone?­7i²Lù?½COJ•ûT?î,‰d±õ?½COJ•ûT?®ã8¬«æ?¿À‰æ{Ó?î̹¸b?¿À‰æ{Ó?Û+\ô'{­?¶ŠüÐã?âjQ…·B*?¶ŠüÐã?Ȑx%ßW?¢°»KN©?éÛáöˆ:ª?¢°»KN©?ŠEÀBi Ç?¢x²Íªê»?ï–èþöY}?¢x²Íªê»?ž3Ñ –?ªãúªša¯?0òwg?ªãúªša¯?Êjb/Uz?´°¶¾›ñ3?éeg}4*¡?´°¶¾›ñ3?'tZ®c?€]΁¸1?ïl]/tÑ}?€]΁¸1PSR3FGL J1013.6-5734@q°ò䎊¿íçù¾ÈR?À8€"¸aÀ:‡dK3'?ü»J}@9[‰"'?ù¯Àéz-?ïÿµÞ¯ßg¿è¹™ÈØ:X¿ëZ®ô¼Å¿äq[ˆ£
rUNASNone@Œ 'RTaLogParabolanone?æ"˜+Žè?Ó Ge.?ӺϨãþ1?Ó Ge.?¶7ígÁ?Àä¿°.°?í9Rô!X?Àä¿°.°?ã>gØ	•?·â#Øï'A?ك0OíÂÕ?·â#Øï'A?ÐÝê_ˆ'?°'*˜¯?ç'
Ðy»¿?°'*˜¯?ÞVûöl>©?×­.ؖÀ²?àԂÉà¬?×­.ؖÀ²?'Ò¿nØ_?«
Ëó"H?ïqo";'ý?«
Ëó"H?Þ?ÖÛªœ\?¿189àÔõ?àà'*±Ò?¿189àÔõ?¥=jÎåW?,8Î?î¬)S,ð?,8ÎMIXED3FGL J1016.5-6034@qÐ=Ć­À	¶	8ÿ%À8¢qȚ8%À:í…AóÀW?ü4_,
@9ΛÙæ@U%o¦+"¿ÕðkhêáF¿íÞ[¦!šã¿è1Xh)'©¿ïþ°ð"g^UNASNone@…1ÅLogParabolanone?ÐVÚ݆®Z?Èe²â?ü?çԒ'<¨Ó?Èe²â?ü?¦¯+®y?¿˜»òù¡?î•
E(?¿˜»òù¡?àèÃDÛ?´
ñŒ52?ßÄ.yvIÅ?´
ñŒ52?¼TI«i·?œ÷œàõˆ?ìuv݊'É?œ÷œàõˆ?¬ÃÕÝ`¦…?´T3	Ìð?î3¡òûØ?´T3	Ìð?‹Þœ¦…Æ?ªë̏Iq?²¡9?ªë̏Iq?מݒåè?»6©§1n?ä0'6tŒ?»6©§1n?‹¼v?+ÌÓ?zx=WêÉ?ï'',Œ?zx=WêÉMIXED3FGL J1026.2-5730@qÆM@$³>? µÐ±Þ´×À7Èn4'EÀ9þ¦-?ÿ¾‰öct@\è"ÿV?ü6ݲMD¬¿çƒ/NĀš¿Þ8I5[µ¿é®
Í{¦ó¿éE狏–UNASNone@œj'ø7´¢LogParabolanone?R¡ñÕ Ø?aT†œ?ïö¯9>/?aT†œ?¨qŠ£/æ?¿bÉ—á?îxçUö<ï?¿bÉ—á?ÈR¼v¤ˆF?±ýX:;«¡?éëPâVÝî?±ýX:;«¡?½'6]t?›ûuST•ø?ìM¼94\²?›ûuST•ø?Fvò•ók?FQŒG–Kº?ïúbX~‹?FQŒG–Kº?‹Øµ6£Ã#?ªèìøm7Ü?+@íÓ?ªèìøm7Ü?¸ÇðïÐz?°ýx^—ë?ìçâi?°ýx^—ë?<Ì-"tŠ?|Ø ϔ?ï‹ςoî?|Ø ϔPSR3FGL J1035.7-6720@r&@·€4nÀPBÛÀ8`
z­EHÀ;?zF;†@'ð4ÛÕ@Í£ÈDŽŽ?ûôÆ/¿Ä€ó·áó¿àG±èDøX¿æۛÙS²ž¿îCRªò²eUNASNone@ˆW:}ªOÊLogParabolanone?4ñd{x*Ÿ?3E]¬´(n?ïýaÓbEÎ?3E]¬´(n?¤6å)C,?¿±ä~š9Ó?®h³ž?¿±ä~š9Ó? ²¹û3Éx?•7b¡?îôÔ`?ù?•7b¡?•cîIƳÞ?x¡Ö>¼"z?ïTàÛ±?x¡Ö>¼"z?;¨,›"[þ?4ÖºÙ!Ò?ïüŠú'Îk?4ÖºÙ!Ò?‹qüûrU?«$déW«?ï'8'7?«$déW«?ˆð!c€m?ƒôŸ|m?ïœ?ÓCx??ƒôŸ|m?`x¯²iX?Pô«ÈÏñ?ïï‡P'?Pô«ÈÏñPSR3FGL J1037.2-6052@qõ"œwškÀT*#¿ùÀ9ûkEÉ8À:õå†6a?ø‡,å'?@
Ââm©Q?þ£ÐqÇîl¿Þ7 <$bO¿ëŒíîÒÓn¿áûÛxê«
¿ïÿÿ¬?…ôUNASNone@'{kjçÕgLogParabolanone?á¶=æYTŸ?×ÃþÅËÚ?ܓ"3MVÂ?×ÃþÅËÚ?³Š~R§~?ÀH™£÷ãÉ?펽P5«?ÀH™£÷ãÉ?⒜R±E?³Ä
½e?ÚÚÇ[ôv?³Ä
½e?ÐÞKaŸ¤˜?§áp«q?çÚO0-´?§áp«q?Õ¤õ3Y"è?Ôȉ¾|ŸZ?å-…fS=Œ?Ôȉ¾|ŸZ?'l¦Ya?­ŸVqüœž?ïw䚖;8?­ŸVqüœž?ÛºS_ÅÚ¸?¸-ÍG	î…?â"ÖP¤?¸-ÍG	î…?£ìüÙ_ Z?'rÐ?
«?îÁ023;?'rÐ?
«MIXED3FGL J1037.9-5843@qåz–¼¿ÌèöÎþÖ4À8T=;"À:c?J˜ª†?ùhðÊ-
O@
Hy|î"?ü]Bf×пæ1QÚúHA¿äl(
Ôèìl†!Rò¿èJGy€
UNASNone@¡Ûgy¦µLogParabolanone?Ï~éÎ?Éo:õ?è »ù?Éo:õ?´ÞµW5?À@^NÜ?í~$)™Æ)?À@^NÜ?âµä¡æÖJ?´¾ƒ´°h?ڔ6¼2Sm?´¾ƒ´°h?ÎÙ?RW?¥àZ²ÎÕÙ?èI°>»kj?¥àZ²ÎÕÙ?˜&%ú'³T?¡«ÐŽ.s´?ï>ÎÐe¼%?¡«ÐŽ.s´?_O!Ï~?­{Ó)¶?ïͽëD?­{Ó)¶?Õ¢‰Ô÷àï?·ç]LÛQª?å.»"ˆ?·ç]LÛQª?™"ˆLe?†ÌUՇ?ï7ë[Ù·?†ÌUՇMIXED3FGL J1039.1-5809@qã4¢3œ?ÖuÌ}ɯÀ8ÖmpEã9À:x‹îN?ùžv*úÕ@ü²ÎHøÂ?÷'\ÆÕfú?ï՘KÌîA¿à'ß\¶(4¿æ£% Bb¿ïÿá…ÓiUNASNone@žSoìVÕÐLogParabolanone?àzÙ®ë7? IõéçêÔ?ïxü)Æ? IõéçêÔ?«¢xelkc?¿pš0m?îEØy©9J?¿pš0m?Ç;f;?®{¤mˆ?ê99þ1&q?®{¤mˆ?ÃÏ{?ˆÎh?¢~ÇQÕä?ë!0Ìf?¢~ÇQÕä?nÀ¡æ-<Â?¢¯ñ¼ô§,?ïá?]ìwë?¢¯ñ¼ô§,?Nÿ•ÂŒ'?ªóÞš3t?ï'ÄÄr®?ªóÞš3t? Ôö`Ò&?˜Ñç÷Û?îò°šϽ?˜Ñç÷Û?•:õµƒ?'EݯÉî?ïS(œ'"?'EݯÉîPSR3FGL J1047.3-6005@r½<64¿ë–eÒ°À8Yóv"Á›À:;°ÂF?øF&ñ}@$	-{8[?ü<|Ã$¿Þ®ØÑñW¿ÄòH'ú¿êÛÞLž` ¿ät+º²²´UNASNone@¡ÊgE8ï5LogParabolanoneT?ÎqEƒ~
ƒ?Ë»§Wêš
?èc®Ÿ }_?Ë»§Wêš
?ÐáË~v'?Ç၇æ$?ç@·Äí?Ç၇æ$?á™ïÕ»^?¹¨G.>¾?ÝðÌ T‰D?¹¨G.>¾?à0 çõ$ã?¯œ\`‹Ø?ߞ¾0¶9?¯œ\`‹Ø?˜áLßÍG«?¤Í5õiÖ?ï8õ™8'?¤Í5õiÖ?Ÿ¿§ñQ½?°X|œGo?ïÀ"rR?°X|œGo?Û*ØÂ_œ¯?»<]ã³?âj"žÐ1©?»<]ã³?¹ãJ…½Í3?§Ð|âW7D?ìÖ¯HFZ?§Ð|âW7DMIXED3FGL J1048.2-5928@qý³Ð|"¶¿Ð¬@$Þ0ÍÀ8Esvð!fÀ:7F°¾yM@…'5yß@¾ÅÍÿý§?úZ¢e›e?ïϯ??¨Y¿Öºèÿ]mÄ¿ëÊÿèƒ¿çoi¡H(}UNASNone@œm¨õ\LogParabolanone?ÛW¦Úõ¯o?×&¥A~¶¥?âT,'…(H?×&¥A~¶¥?©<w:Û.v?¿"Íyglm?îl8ŒRM?¿"Íyglm?Ó¬¥v,é(?´ÊãOCÊ?æ)­Dé‹l?´ÊãOCÊ?Àqé×Â?¥àNçr)8?ëã›Ø…Š?¥àNçr)8?Àh®me<?ÍÒ]–šG?ëåÔ~$¦±?ÍÒ]–šG?KJíiCs?«¾¨:Ôå?ï}¥¨y9?«¾¨:Ôå?Ø8ààï³F?¸'G…n¢?ã㏏ˆ&]?¸'G…n¢? PzÁ½$?•ñ@£‡?îÿøSä.?•ñ@£‡PSR3FGL J1056.7-5853@r	7ޓž®?粓€zä£À82Òò€»|À:°†ˆD݀@ð+Voù@š@QT?ýaÿI ÛB¿Éb_CF¿åÌ<>Ó-¿ëå­X_´é¿ïÿ¡Ïý6UNASNone@FØ_ö"LogParabolanone?uÿL§$¨ö?66Û¤Ð?ïÔf~Üv?66Û¤Ð?¢iìÔeX±?¿˜Ó\D?îÙa2þb¥?¿˜Ó\D?Å~…›'t?°©Ë‹œ:?ê ^¸Ù6#?°©Ë‹œ:?}Ü¥Ñ?bŠ"wö?ïÅF¡è?bŠ"wö?ƒÃR•n$Â?©Ñdg/©?ï°òµ®fõ?©Ñdg/©?ˆÚdþ°•?ªôϺÜÃ?ÂBÉî?ªôϺÜÃ?³ûj+›Mõ?¨6"¢ËØ?퀒ºµÑ'?¨6"¢ËØ?@;¦«²Ï?3»#]Ù&?ïûñqö+?3»#]Ù&PSR3FGL J1104.9-6036@r#¹#¢œx¿ØæØ|-xÀ8脹7ÅÀ:~¤™@3gáe¶@l\õyi?øáY÷˜'?ïÿX"ò2¿Ü-vÕ8E¿æ
L|/{n¿ï~@ÝÀºñUNASNone@Ÿ-ñø .LogParabolanone?	Âüàº7?¤Âtaùî?ïÿ˜ôO•?¤Âtaùî?£<Ƀ=?¿"U÷r+°?îÌ3géü¼?¿"U÷r+°?ŽÜá¯íIî?'QyŸr.m?y‰?'QyŸr.m?œß¦ðÏsa?'Ú¶êjF
?ïȇBÕ?'Ú¶êjF
?*;䋔CH?.'#û±ë>?ïþ\AÒæË?.'#û±ë>?ŠPÒÌ\?ªòt5F
?¼‹"§?ªòt5F
?}ìß:-ex?†Ûž‡ü…?ïÄ&Aw?†Ûž‡ü…?s	mAïà?cÚI†ì?ïÙí%v à?cÚI†ìPSR3FGL J1112.0-6135@r6^Ý)5¿î¨0 ±»ÏÀ7Ù³×2]À:C6nQs@«húp@Έc¼=?þ#ÉO"¾¿ÑåÅÊ­–¿æôþǛµ¿è]—ÆìÊ¿í£ç?·"UNASNone@".1&éyLogParabolanone@?RiúÊ9?gœOô5y»?ïöËq`ž?gœOô5y»?£ó/ÐÍg?¿‡ìæü+"?îÀÍãÆJ?¿‡ìæü+"?ÅO¹Ȫ?¯|VÀ:Ÿ?ꬺMÕ\?¯|VÀ:Ÿ?§k¬Ãá?‰túbcÖ?î‰E?
"?‰túbcÖ?h‹ÁÏ\?q»#}@Ç?ïçt>§kÐ?q»#}@Ç?Š³¦?'<?ªïHEë¦ë?1K…?ªïHEë¦ë?Ã(Û‡"Æ?´`CnŒ%?ë5É>^Ï?´`CnŒ%?z¶Ûáu?jhsÎ?ïËÇèr«Õ?jhsÎPSR3FGL J1119.9-2204@qGƒ[Õì@B†6`åÀ8Ώљ»(À;™tÆ{yô@$7÷E¨@Œgƒò¾N?ö
óxˆ'¿¥øV9]¿ß,âP–¿è Âb(‹¿ïÿê#¨YYUNASNone@ˆ½ª šª;LogParabolanone?…~8ð*'²?"SóÿÒ?ïªvOµ?"SóÿÒ?·–O
̳?Æ=Q±*?í
6u?Æ=Q±*?¾"vTTÊ?© 3Vbšü?ì-q>uug?© 3Vbšü?™ÓÓTºè*?€!l囸?ï1ae0ío?€!l囸?{Fq}˜?"Q菦r?ïÉsÊä%•?"Q菦r?¤>Vsqj:?º7‡ŸÝ£?»*ì?º7‡ŸÝ£?¼»?^Ì?¯pŏµ¢?ìhn'?¯pŏµ¢?c¤–®Êܜ?RÜYS³9?ïì[iCv³?RÜYS³9PSR3FGL J1120.6+0713@oqÝDU@NW´NPÅëÀ9ÒñÑsûÀ;åû¤P¬Á?úèE‰L‰@þEjÃB_?ñ›±‰¥ZÃ?ïKT
¡Í¿Þ~G˓R¿äH§Á¥|Q¿îÃËV€bUNASNone@"k›ÚQÎLogParabolanone?ºÕ_áo¤±?ÁXdÈ#I?ì¥TÒj?ÁXdÈ#I?ٚ0+۔Õ?Ï	é"f?ã2çê5•?Ï	é"f?ÒziQñ?´Mmš?æÂýKxW?´Mmš?Ùä+ÃÓ)?²+,z¡G?ã
êk|?²+,z¡G?¦{jÍñ­?²U»"úü?î˜I_Åbu?²U»"úü?ÈÊÅp•?Ë\¢>w?éÍxN£Ú™?Ë\¢>w?Ê;	ê±?»Žèí?éq9}œ…T?»Žèí?¶ÌDwåP? +Ôøz×?í0w,K&? +Ôøz×PSR3FGL J1128.6-5434@r0˜ñ/@z	Ì1œZÀ9eDܨâãÀ;cÚTtÌ[?÷9ÞóëË@
M¢÷Œ¿@
l…E¤¥¿á×i'òÛw¿ë+fiþ¿ïØڌï¿ïÂ
H½ÞóUNASNone@tû‹C•LogParabolanone?Ñͺ[c±‰?Ǘ>‹#¼?ç"ÒN'<?Ǘ>‹#¼?¯®ÌÍÓÐ?Âi™"ó—^?î3I¿£?Âi™"ó—^?ç{Wº&,?°+døF0
?Ñû	P‹³¨?°+døF0
?ÁÄ.X-³?¤h¯}è5?ëŽôiô»S?¤h¯}è5?Î|€܊¹?Ê'å•N8ü?è`ßýÝR?Ê'å•N8ü?"ßߺjhŒ?°î$	ši•?ïa/Ü?°î$	ši•?àEdǪÏ?¼sÈqâˆ?ßuã6pªb?¼sÈqâˆ?'¡N%?vÁ†ž›[?ï´AquŸP?vÁ†ž›[MIXED3FGL J1128.7-6232@rYŸ±¿òÓe7'=…À8º5À¬-À:¶î#;n?ûó"vøYî@|CÐd[õ?ù!֙Õ(¼?ïô`9¦"Õ¿è:5+Âå¿êg…î
‡¿åáe<3¦ºUNASNone@"L¾ùÛ"ÑLogParabolanone?ÝÂ!Î×?ÒS7%—Oy?áïüü?ÒS7%—Oy?¶VÝñ?À½æ(àÁ?í5<L?À½æ(àÁ?äm6Ý{Š?·îJ<Ðp?×%גEë?·îJ<Ðp?ÑQyW¸VQ?¯jºñÉ'?çWCT#ÔØ?¯jºñÉ'?Âw
¹cÜ?Äë™>ˆ"|?ëb?½Q§	?Äë™>ˆ"|?'ü1$¡[@?«ó_˧?ïpw­V?«ó_˧?àu¤<{ ?¾ìw¯[o4?߷χÀ?¾ìw¯[o4?¦'%4¢1?›¥OŒ-–?¬ÑYÏ?›¥OŒ-–MIXED3FGL J1208.4-6239@r ]'ýuâ¿É¿{*˜°À8ô!-wÀ:	÷;5`4?üJ5XQ@©·6ì%?ö̼†®…d?éòz1Ìß¿ÖÀ}xü–¿å®€Rî¿í§õ'ùoUNASNone@ ÓbZîc LogParabolanone?|q̣Ÿp?>
½ù>S?ïÇf½ú!?>
½ù>S?»çn½ç›t?Á6œÇÿç	?ìƒ(C'?Á6œÇÿç	?¾0cõó·?ª¦ù7ùf?ì9óA‰?ª¦ù7ùf?Ô¨yV@!?®Ŧóc?å«ÃTþßï?®Ŧóc?L×ñ_
.˜?SQ¥Ÿ»_?ïøÊnÊc?SQ¥Ÿ»_?ã8Î75?­JEózº?ïæ;Öf?­JEózº?›VuRs‡?ŸùkâcÐ?ï%LUC(t?ŸùkâcÐ?¶õ?³çQ?¡l€Ï¢?í!X	¬Q,?¡l€Ï¢PSR3FGL J1225.9+2953@g$ÞÊl @Tðñ¾ôœõÀ9wÒ4jkÀ;¨Öí·ÿ?úOó«³Í@>¥"8äù?óJCðð™?ÒïXæ© U¿àW¼ãÜÄù¿×UXÂ8õ¿ì'ŠyÉ£*UNASNone@›YW$tSLogParabolanone?®%Ê}»Ù?±d~‰yº!?î£^5â²?±d~‰yº!?ÜûìjKù(?ÒׂŠ€ÄX?á'	ÊÚl?ÒׂŠ€ÄX?Í¡\_ì§?²P€3❩?藨èûV?²P€3❩?ڋüt҇C?²i$žÕIœ?âºŖ¼^?²i$žÕIœ?‡.VsŒç?ŠbRŒh#m?ï£F¦$
ô?ŠbRŒh#m?ÑçEF䞃?ӕ‹"g•?ç]\°¾?ӕ‹"g•?ƶÛó?³1.4~‰^?ê{¹ÒI8ƒ?³1.4~‰^?¼Éí|ù-†?§)Ñ&ýœ?ìfÂP`ÚO?§)Ñ&ýœPSR3FGL J1231.6-5113@r¼Aò×s@'»%}À9fƒÂ—ÀÀ;uëGWL?ûšÄÒW{<@ĂLuúX@ó¡­k¿Õ:æÄ*ù¿èAܕ†~N¿ï礉·¤G¿ïØ¡—>ö`UNASNone@|fË}At?LogParabolanone?»ß÷ï1Èò?À?+>6
?ì"Æâ?À?+>6
?«»Ì­à7?ÀìJòÓ­Î?îDC4÷È=?ÀìJòÓ­Î?áKgpì@?´½ýÅöÁ?Ýi1'Ã?´½ýÅöÁ?²ý˜"Œ:b?'/í÷¼?í Lï¥rs?'/í÷¼?°IjËÄi?½¿šÃ÷L?íöÒ¼L#?½¿šÃ÷L?''¬+‡¯?«r6B¯?ïnž~8s?«r6B¯?Ûbîž}?·§]0x<?âNˆô°Á~?·§]0x<?rÕò4@G?aiº(d^?ïÛúSåý˜?aiº(d^MIXED3FGL J1306.4-6043@sKœ¶"Œ@±]''À8xÅ
»ªÀ:¶…F%~??ÿƒ>ùºì{@™;³4uS?õrjùs¿º¯&&bóÉ¿Ößë}ù¿àì6GöÊÞ¿ësiø¥²UNASNone@˜>Á$Ý/LogParabolanone?=L½"|Ã?Iðš¥Ç?ïüV|°Í	?Iðš¥Ç?£h¿èE?¿R$ÝQw?îÉwÑ|?¿R$ÝQw?µÕ™w
gB?¦èæ°d•?íELÑGŽh?¦èæ°d•? 2¶Q.rŽ?µ¸ï'QÒ?îüԛ•·?µ¸ï'QÒ?MErä'[Ç?Gz­	lš?ïø®£±$?Gz­	lš?‰½†b›v?ªñ'r·›?ï™	ç½òr?ªñ'r·›?‰Geys?‰]–Z¶4#?â‡bú?‰]–Z¶4#?lÈtR¢æ?[,B£õ…V?ïã7àlõ?[,B£õ…VPSR3FGL J1317.6-6315@sñ¾ôœõ¿á3Ïp;ÑÀ8?M«"}©À:g"©GŒ‡?ù9í|o½'@a'ÇMµ?ûJ)©ò'>?ïêu^üº¦¿ã^,æ#é¿è&lX÷F¿îgùt±¾æUNASNone@œúÁ‰7KÇLogParabolanone?È0æIÍ?"\³ddç2?ïˆß?É¢)?"\³ddç2?²ãÝj۔?À•ßèTßù?í£œdªÎ?À•ßèTßù?Ë`áVnjò?°"Ë—D‹?é'ǪNÄ?°"Ë—D‹?Î7Ún~–?¨ÁÝ<P?èr8	d`Z?¨ÁÝ<P?Jq°¹Ÿ20?Màó?¬œ|?ïùc"Î(—?Màó?¬œ|?"(Z¡"?«#
MÕÒ®?ïf½*å©4?«#
MÕÒ®?š´}™µ}Ž?•eEhà?ï*\@ƒ?•eEhà?£lrº˜Ô?Žên¾ç–Y?îÉ6ù¢?Žên¾ç–YPSR3FGL J1329.8-6109@s8ҝÇ%Ä?õÕ`IôÀ8ÔG'‡|À:€ŠÔÚ¸?øBw÷]o@Åßó›?÷pµµ.£¿Gctö/¿ÝÓÙ"à¿âõ‡›D¿î¼P3°AãUNASNone@˜¸²a|ÚLogParabolanone?™Âjú'?¡æ1é|?ï1ïä~ð ?¡æ1é|?É'SØwÙ?Âü[/Ñ~ã?鹫	â
?Âü[/Ñ~ã?ÓªY'9ö=?²§ÎߣH'?æ*Ó6ãá?²§ÎߣH'?ܐç'…Ä¿?«ii»…|¬?᷌l= ?«ii»…|¬?d1Æ|s¿{?f'¤3äš?ïëÎ9€Ì'?f'¤3äš?žsíáMž?­Ðå#DxŒ?ï`—U­Ã?­Ðå#DxŒ?­*üñÂJt?¢P%^î©À?î-P0Öé?¢P%^î©À?ºZ:…
_? ´ÃðÉðé?ì´¸¾o^T? ´ÃðÉðéPSR3FGL J1350.4-6224@s[ZîcŠ¿Ôy4¿zSÙÀ8i1ÈÏè
À:sî,ëñ?ý"£'–Æ@B%±ŽX?çµçF[ë?ïúT\ü¿Ñ¿•_V¿â"°õ·¿ïÿò|ðÒ¢UNASNone@£%¥¼£nLogParabolanone?p©	9<Ê$?')P_ùA?ïÞ­í¹k?')P_ùA?³Å¿~!òX?ÀªÐ-j?í‡Hdý?ÀªÐ-j?¶-î%ð§?¦½
ÙZÅa?í:\›?¦½
ÙZÅa?ÊÂI`ØC?«þ›°ó?éO}í§Éï?«þ›°ó?'Ê>ínŠ?« -¨÷ß?ï·¨ÖÖïn?« -¨÷ß?—[g£µù¸?¬|Tk?ïE$Ë'?¬|Tk?ž‡þâT»?œÆقb§\?ïÀ	×?œÆقb§\?¨³ƒ?"}?˜`ggÐñ5?îtÇèˆ?˜`ggÐñ5PSR3FGL J1358.5-6025@sr	ԕ+?õè|4gÀ7䐴Ê!À:Sýå¶?ûI"dvL8@Éf<J7@Çþ†Ù#¿ÒVƒ¾Õ­
¿ä˜Ñ1$T¿è'&›É¿ï-9†ßW¿UNASNone@‰Ñë…¸LogParabolanone?ƒÝS,;d?'p÷zU1?ﰊ³×?'p÷zU1?©¤¥a/6?ÀæažU–?îeµª$ü?ÀæažU–?Æ1ƃ::?¯•GñÎgk?ês¹Ž_1q?¯•GñÎgk?Áö,Èò?›Ó¥ëÕ4?ë'tÍÃ~?›Ó¥ëÕ4?@'«Ã­f?C~ö>`Ķ?ïû۔Õ~f?C~ö>`Ķ?ç3eë?ªç©‹¼þ?ï‹Äc
«?ªç©‹¼þ?•¿Ñk>›?"ok¡"?ïRwy^;?"ok¡"?''U˜1?zÐl¾i¬?ïvÇUD¸?zÐl¾i¬PSR3FGL J1405.4-6119@s{!Bp?ҕa¼­žÀ7Ґ[,À9Ëp£×
=?ÿñ´â@BüŒX'?þ_ÛÛ£
¿Ó‹
9ÏYš¿ä]ï֫⋿çvº 5¦;¿ç"vµû
^UNASNone@ ÏRn—PLogParabolanone?tžI{!õû?z~K,Ÿ«b?ïÖÃlë"?z~K,Ÿ«b?¤È'~¼+?¿|ÃÏ<¨?î³~æ¡~?¿|ÃÏ<¨?Ð)¿*ä°?²ð 1Pi?çë tꍨ?²ð 1Pi?°…ƒJîRé?'fûén8Û?íïO–k;ã?'fûén8Û?sîyˆœ?":û$ã2?ïØ#Ó§?":û$ã2?ŠŠ®îó?ªíƒ…öh?ï•×ÅE¼D?ªíƒ…öh?Ò€eô")?¹°vø&d?æþ?ͽë?¹°vø&d?~œ[?nw´i¿?ïÃÞÇK-¦?nw´i¿PSR3FGL J1411.8-5743@s˜•1ã¨@èX¡ÅgÀ8õil«$À;Î70ö?øº¢OÎ@'9"áV@áÈ¿Ì߿ŧä•o¿ë·Ö¡-¿æ[8'R3¿é†¤9ä/óUNASNone@'9¥zxl"LogParabolanone?·û/?Çþ'âÆ3V?è^>Á´??Çþ'âÆ3V?´×7<øÆà?À·ðǨÌ?íen¥"?À·ðǨÌ?ç¦7g(?±g¯äƒ?г͑1¯ê?±g¯äƒ?ÒÙ¡NP¨?§®×³•?æ"/X÷׬?§®×³•?¯MG¿-é"?³2»Až¬?î+ƒÖ'®?³2»Až¬?'ßÔ4¡Ó?­žÒrÚç?ïoÙla?­žÒrÚç?Üä½¹¶"?»«ÓSµÅÛ?፡|£$ï?»«ÓSµÅÛ?£Ãß
M7Å?H+wXû:?îÃÂb&C?H+wXû:MIXED3FGL J1412.3-6635@sm¹à`þHÀê°]*}'À9†ŽVox^À;@ï›2÷?÷U¸ìp+6@ò©nοÁ?ú2IÂ°¿Ýy¶rËØ¿âi·š›¿åœ0õì*á¿ïÿéåèUNASNone@"TØ_ö"LogParabolanone?Ín7Ç}¾®?È̘K³)/?è¤r U?È̘K³)/?Å0êX£Û?ÂûÂG|…&?ê³Åi×	<?ÂûÂG|…&?á'¢
h?³p¤ò'ç?ÝâÚÞ»ë1?³p¤ò'ç?ÙJ¡OÆg?¬Äéò€G?ãZž¯XÍ?¬Äéò€G?Ž
r¤û1?›–Ñ9ÚF|?ï‡Ê5‡?›–Ñ9ÚF|?—ç·T'°?¯]HC[aŠ?ï@ÂE'äÒ?¯]HC[aŠ?¹2߀w—c?§3ãRw?ìÙ¤‰ô?§3ãRw?®ÓuÆFD	?˜Àz{h£z?îÈ£·Ÿ?˜Àz{h£zMIXED3FGL J1447.3-5800@sÜï4Ö¡b?÷®ITèRÀ7ÿö¶«"XÀ:…Ћž.T?÷¢!Ódk@'
t­@Ýë´½·¿ã€ÌÝØ|¿éy<˜üT"¿ëøcb"¹z¿ê¹ËÌ$cëUNASNone@u.ã^J8LogParabolanone?Ò¨sI¬O?Éîâ'B˜?æ«Æ[)Ø}?Éîâ'B˜?µ¡›"v	?ÁNiûi¾?íK̏:E ?ÁNiûi¾?äbñÅæºÆ?¶°F5AËê?×:t2Št?¶°F5AËê?ҙ©Ó´¯?©"³Å^?æ³|+%©?©"³Å^?­¢2fÑé?µˆ';œõ?î/uÜْá?µˆ';œõ?'sÈSà4°?¯äÒ
d¨²?ïla½Š9ª?¯äÒ
d¨²?ÌöC`p?½žN¶V?èú'o'ød?½žN¶V? O¶0/?S_YŸ*?îûœá'o?S_YŸ*MIXED3FGL J1456.7-6046@sÚVlô!¿ø˜}õÏ$–À8I)B©DÀ:.^¸<?ûCç@ìY@"óoMì@'åÆmã¿Ãö'àªáQ¿ë^}õàS¿ì"f›YQ¿ì17î-ð~UNASNone@D;Í5¨XLogParabolanone?y™
ʬ?fˆVB…J?ïÌÍËÐM‹?fˆVB…J?°Î¯À(wä?À[µNg'h?íæ*¯s?À[µNg'h?Ôt¢Xè?²½vÍϜ¯?åûÅ®Óñ?²½vÍϜ¯?ÍQ2"åX?ª+Q?Qn?諳žÆª?ª+Q?Qn?n¼1Râ?'·¡Ï %?ïáCÏ,?'·¡Ï %?Ëÿ®À?­¥Du4fb?ïy§Çëͪ?­¥Du4fb?Î ÀŠQz?·ÏO$~°!?èwÏÝxk¢?·ÏO$~°!? 'ò±C÷?'{ÓÔá•È?îöÐÕ"ºH?'{ÓÔá•ÈPSR3FGL J1503.5-5801@sûX£/D'?Þ7_úfŽÀ8–—†™ãÀ:5œBÁE°?ù§œSÞ#Œ@Øٗ
ž?þH»eqHî¿Úù> #Ìc¿æòn-@f¿æ¯'ùš¾»¿îڌ{×oqUNASNone@–Ëzxl"hLogParabolanone?ÁîÓù¢ÿÛ?ÄWÙI¡£?ë"K—@	?ÄWÙI¡£?DžŽ¸ô?©`möJ?ê¼Ï\QÃ?©`möJ?Û̒⒩2?·–bMA?ⶎ¶«g?·–bMA?ÛÒUüû'‡?«P1j¶?âÕ'>½?«P1j¶?èßÁû*?šÕVåé?ïˆ\ƒÊ¶ƒ?šÕVåé?œ"_\ ®¦?®!ÿ£ ?ïeÖB[?®!ÿ£ ?ÌØ{ÆcÀÞ?´åØÒu o?èÉágÈ?´åØÒu o?¸˜ÓñMB{? Þf¤»?ìì偭a? Þf¤»PSR3FGL J1528.3-5836@t"»â.]á¿û"à¢l¦òÀ9~e`¬éÀ;_Þ+™á¾?ý}©^2»>@ë.QL#¿ã–/—ÐÊ;¿Ö؎ŠO'R¿¤ëÄüÍ/C¿æ!ڛB¿ïÿÇí%CUNASNone@ Ÿ§ï²LogParabolanone?ãOQr%?Ùy k
Ò?Ùa]Ó´â?Ùy k
Ò?БÇûN6ç?жqãêm?ç·XäŒ?жqãêm?Ê·Oü±?°§&Î`?é{y',Ô?°§&Î`?ÑBŽ)àí?¼,Z€Bõ7?ç^¸ëwŠ?¼,Z€Bõ7?ÕÑ,•+Ã?Ú½úóŒæ>?åiµjq?Ú½úóŒæ>?¥=z*…¾?¶š˜u(âR?î¬(]Iå°?¶š˜u(âR?ÄtâM	?´òÔáRÇ¡?êâû‡l½»?´òÔáRÇ¡?¢Å½ÇÏ9?£dÞQ¨¬?îÓ¤#O)M?£dÞQ¨¬MIXED3FGL J1539.2-3324@u,%ãS÷Ï@1ˆÁDŽPÀ9.èŒEôÀ;š^x[[p@(Ò·rrŽ@;«Ò(+¿ó…¦÷ú"?ïþ°Q/â?ç¡eº]Î+¿Ü>S"ø䔿í‰ÕB€òÈUNASNone@¢›~ùÛ"ÑLogParabolanone?Éóožs?Òº¦˜õH±?éƒ>;$c?Òº¦˜õH±?¶Ê榸ï?Ãd£ǜâ?í&£=á?Ãd£ǜâ?»
ÛY?¨'5¶R?ìœÜü^¤•?¨'5¶R?¬<ÍYÈDé? ëö*
¸?î<3*,ò? ëö*
¸?ÊgÊ\¸›E?Öüu™+¬ù?éf
hÑÙ/?Öüu™+¬ù?¥¹UTù?·ƒœ×¤‡­?î¤j¯¤p?·ƒœ×¤‡­?¼'ó¨Èzq?±@|Á`vÒ?ì{Šæð²?±@|Á`vÒ?† ¬|ƒ?‰ÝpEþ¶?ï§~@O"?‰ÝpEþ¶PSR3FGL J1543.5-0244@K¯'9*Ä@Cs7âÅ\–À9ÀÁœ¬tÀ;¬U^f?ö|»WYƒ)@±¦˜/·(?þG;N	οҙÎeܱO¿âÞÓüýþ¿ëù+'Lm¿ïÿ¨×¥ýUNASNone@‹"£9ÀëîLogParabolanone?禯Xa"Ä?ËÈ:R"?в¡O<öx?ËÈ:R"?䉸ÃÝ?Òí3˚®Ô?×ÔìúxE?Òí3˚®Ô?åwwþ"E?²¨Å@p€?Õ×uÈ?²¨Å@p€?â~°¡6à¬?°þãuȾ|?Ûž½'>©?°þãuȾ|?ÌCÞ7i‰î?Èä"‹½…T?èïr%…?Èä"‹½…T?Ñ£E q?Óz¼ðÇäí?ç.?s]oÈ?Óz¼ðÇäí?Õ`'ª`^?ºé³"ÛÈ?åyÏì*ÏÑ?ºé³"ÛÈ?¾Lï¥rsn?¥"ÚÜÙ*?ì6bQ±'?¥"ÚÜÙ*MIXED3FGL J1552.8-5330@t]$žDú?ÓkM
ìÓÀ7å-c™ÑÀ9ùt,!Æú?ÿþnÞ,µ@´Š­B˜×?óÕ7‡€½U?ïÿŠºZH¿Û+4*©ø¿ã¯wuhž
¿ïò]΃AUNASNone@ h€IRLogParabolanone@?!"ûLü¦?4XÔ¾Å+?ïþæ°"È?4XÔ¾Å+?¤úBhê¬?¿ƒ-\¶ï?î°[ÙUØ`?¿ƒ-\¶ï?"¿ç°)³@?"–M{à€?ïbŒpÖ?"–M{à€?¯*W *£?"U0pòB?î
ZŽ
kÆ?"U0pòB?Oÿ†X
Ñ?}v`6#?ïø;Üq}?}v`6#?ŒŒQ‡‡?ªï£gRéj?òr?ªï£gRéj?'F–̼"÷?™
áÀAà?ïmËIŒ]h?™
áÀAà?†Éo³Ì$?vôhcõC?ï¤ÚAgð?vôhcõCPSR3FGL J1557.0-4225@túB¤TÞ@ ¹mmÁ¤{À8ÔÔ{øÀ;
Ìhù¾?÷ÇV%{˜@þý~Ԝ@HåY‹Œ'¿ä Ä+q%¿ë[4aº
¿èM9Þaä¿ïÿT,ÉFUNASNone@wõ£KÜLogParabolanone?Þí9˜–Ô?ÊF´ák?àÿ	c3´–?ÊF´ák?µ®¶{ñuË?˜섑ä]?íJ)0N&?˜섑ä]?è‹K´D§?¯ ÿ??ÏõÒÑ.íe?¯ ÿ??Í%jó"?¥E?Ej?è¸y¶¥C?¥E?Ej?ÂÔÖN´Kª?ÁÐÍ, ?ëJÊlRí?ÁÐÍ, ?šGxV×;á?³Gfï«ÒŠ?ï-Ä= 
Ñ?³Gfï«ÒŠ?Ü$jî`pX?¾€0|tš²?áíʈÏÇÔ?¾€0|tš²?™üVBÐâ?ƒXœé,ñ?ï7Ð[§é?ƒXœé,ñMIXED3FGL J1601.9+2306@CDÙê¦Ò@Gx($xÀ:_ñ÷ÿ€~À<@žReþb?÷6(¦I€@ÎÝћ¿¿Ûäúr™Çß¿èÅ&õ?Îkƒb0ÝÕ¿çD uRº¿ïûõú KUNASNone@œxå`A‰LogParabolanone?ã|{ë!»?Ú=PC z?ÙÅ)¼‰?Ú=PC z?â¥ÒF«­e?ÕUû»LÈ?Ú´[r¨¥6?ÕUû»LÈ?ۜŸk²?»Ú?ÀÏt?â1ù°8J'?»Ú?ÀÏt?×}oÂZ®?ÁwÑNLûB?ätAHÒ©?ÁwÑNLûB?×Z¤Ðž,j?Úø'f´ë?äR­—°éË?Úø'f´ë?ÐAÙ,?Ô';Ùš?çßvüió?Ô';Ùš?̦>Ì!3à?º't`á(?èÖpL÷³?º't`á(?¢Ø¹°‰vì?¢ñøG¨IÛ?îÒteåq?¢ñøG¨IÛMIXED3FGL J1622.9-5004@tÛMüã¿Ñíþ`BµÝÀ7nœwškQÀ9ïÇßþù@ T¬)¿@ö¡æÅ~?ò¬œ2Ñ
¤?ïþ¼ö\í¿ÓfIyàZ¿á">‡ïø¿èªs£UNASNone@¥½$Âø7µLogParabolanone?Š«^àðõ?•
ÞÃSÙ?ï•R…''|?•
ÞÃSÙ?©÷þ¶¡3¹?¿Ç§k`Ç?î`€Ú¤ô?¿Ç§k`Ç?Ê·ëçøªÕ?±Ö{Á'=!?éRÕK?±Ö{Á'=!?Àۆ)‹zÙ?¢Êi˜~??ëÉu!J?¢Êi˜~??‡BÈñXÄÔ?'0—®Ç?ï¢ôÜ,Þ}?'0—®Ç?'&ö ±?«9†®ïè?ïvÈJÿO"?«9†®ïè?ÔÏa҂ï3?¹%nžã[?å˜O¾ˆf?¹%nžã[?¡Ô^]¢?‡Ïlº=~?îF?‡Ïlº=~PSR3FGL J1624.1-4700@u•¿ðEx?û«>ËÌÀ7öك"t—À:ƒèäö@ÏM%²—@eý€ò"@¬.õ5÷‰¿àHÅ]0¡w¿î6ý'½\l¿àY®eƒ'¿ê:"39EúUNASNone@{pŠÚ¹õZLogParabolanone? Ì6žÔjF?§}ƙÝk?îó<–;ô«?§}ƙÝk?¤Ò"ïΣ?¿åølI?î²×¿ÞÁ†?¿åølI?ÝX†0}˜©?µ‡"$ãÚÈ?áS¼çÁ3«?µ‡"$ãÚÈ?³`£Ú'bÌ?œdãO2R?í"ë"ÈÒ?œdãO2R?±Û»T¹Ç‹?·™ßîö>÷?íĈ•1ÍO?·™ßîö>÷?‹€å¢ït;?ªæÛo;œð?ï'üi}?ªæÛo;œð?ÓàÌ*‡à?¸®ëUòým?æ|™ê¼?¸®ëUòým?'9¸ÞXer?‡Þ'~`]W?ïv29
<Ô?‡Þ'~`]WPSR3FGL J1624.2-4041@uI&Á½¥@'x³puÀ8f­VœÀ:Â(4Òo¤?ÿØþÑ×£•@l%y6LÃ?õep•x?—{^èV¿à^]eX@Ö¿å…2ƞ¿î±Èe› "UNASNone@";.Hè§LogParabolanone?@,ÿs?×?Ge¡N'®?ïûôÀ[Ð5?Ge¡N'®?¨N×ê½A¢?¿³Tã~Œo?î{2&?¿³Tã~Œo?§øS¬XÉ??ÜÃÊ?î€zÅ6Ó??ÜÃÊ?²
Þ¼˜µ?'ÂX7v$O?í¾žD_f©?'ÂX7v$O?BÏ)\¾q"??ba6'Þ?ïûL5§pŒ??ba6'Þ?'^[ހ±õ?«›‰J r'?ïu
!úp?«›‰J r'?Þ(åˆw·?3:‡á?ïy¸ï9"?3:‡á?ÙgÒB?pÕ3.¦À?︚c¡˜Ÿ?pÕ3.¦ÀPSR3FGL J1625.1-0021@+Âþ`Ï6@?Özúr!†À8¸@ƒ}ÎbÀ;ež8dË\@+ÐïòÝ@ô?ß n?é…ìï_§c¿ËUO
¿½­mÌaB¿äãaó Yοï¯8gOšUNASNone@'.û~ÿ—LogParabolanone?s+‹á!?!Ò¿ø\?ïÿ,fÌxû?!Ò¿ø\?ÁE7,<?Ð5£ÁÌϸ?뮲4ðø{?Ð5£ÁÌϸ?¨«¿LˆN? ¾¦‰Q?îuN4&´[? ¾¦‰Q?:†'F[ü?k¾F-?ï»åÅl0?k¾F-?<²eqä"Ò?4Å$÷2ê&?ïüi³€~?4Å$÷2ê&?ªýɼCŠ?ÅPà˜0¹?îP#d;Ç_?ÅPà˜0¹?¥çîrV7.?¡ 7:Ñ?–M?¡ 7:Ñ?G"ȳ:e?9f­üډ?ïúÍ®Ÿ?9f­üډPSR3FGL J1626.3-4406@u%øa¦
E@ْ]e5åÀ8®•Í\>ÅÀ:lñý2Æ?÷Q¾SEÎ@
lÞÃo¾@(qrÂÀ?à¾ñ¢šO¿îÍfØ°7¿¹4xJZm¿ïÿ¬Lh}1UNASNone@€ß~($LogParabolanone
?Ë_ÒDþ.;?É(ÄýÝ?é(nÀtq?É(ÄýÝ?¹O^Vk?Ä)À½8Éå?ìÞvP¼R?Ä)À½8Éå?ÜóÆNŒ¾?´°ª£ÊM€?á†عü!?´°ª£ÊM€?ÙX6Ìð£?¼øU&M½?ãSä÷™‡¯?¼øU&M½?½ž)(öÌÙ?ëŏ°{w?ìL:Úá&e?ëŏ°{w?£<DU¥?¶g—Ùnÿd?îÏØV?¶g—Ùnÿd?ÛÿŸTf?¶Ìvp€¹?ây€0UÍ?¶Ìvp€¹?Ì_
°ÛH?Iå?èè=Sü	.?IåPSR3FGL J1641.5-5319@tԻ¹M"Àh†
 zÀ8·Â,_Ú[À:Òð§h[?ü–$,?Ö@ªJkÞö?ÿā6÷8¿å`ý6ÞÀ¿â$¿²²ð-¿ë¥ÄD_w׿ïÿ†™v'UNASNone@‰Ó:áG®LogParabolanone?°ü
ÿ—¸?´¾"ªÊ'?íþ`~×É?´¾"ªÊ'?­	
/wʎ?À#Äé‡ N?î/o]AÇ?À#Äé‡ N?×ì¸J3ÕÅ?¶N+od'?ä	£Úæ?¶N+od'?Ã=7Ž6¹û? £ŠÃ\?ë0²rQ? £ŠÃ\?els-b¦v?È×Ùsî?ï꓌E?È×Ùsî?þj &³j?­hð‰‰d?ï€We2?­hð‰‰d?³&>‡i??¤¦N~€H?í›8/ßx?¤¦N~€H?X"òA}-?}ÆûSRJk?t}+?}ÆûSRJkPSR3FGL J1643.6-5002@tÿ÷—|À"¬_nû`À8Ì£²!OÜÀ:©>Ò£¦?û:"ˆ¹@tš{ìµu@ƒ@;ÚL¿ÐväÎKR¿æ
vrf鈿ï4·¬¡€¿ÍˆV8¤iàUNASNone@†ôþÿ—$LogParabolanone?ãÀ"?ñU?ÑþjM?"?Ø~׀áV?ÑþjM?"?à©>Ú4'?Ôa¥È3@?Þ­'KÁ–Û?Ôa¥È3@?ç8¿5yMc?µdu¯7Ä?ю•
e;?µdu¯7Ä?çÒ>ŒéÄ?¶‹	ÌÇ[?Ñà['æ,x?¶‹	ÌÇ[?Úþ'o§úþ?Ô{¹v{(ã?â€ìH,?Ô{¹v{(ã?²Œ¥¹dD‹?Á;I~Ä?í®kI
q.?Á;I~Ä?ä7Ž‰g"±?¹']¦1).?אâí0֞?¹']¦1).?Î KÏâ+?ÅXŠ"²ÃÑ?è÷íu?ÅXŠ"²ÃÑMIXED3FGL J1645.7-2149@vay=Ùc@.D£çÑ5À9'E«Û»}À;om¿öûu?úôõj¥»;@ç²ãA®K?ðž)¶²¯¿Ç¯¾(''¿àuIó`Â¿éï¦Ä$‡Ÿ¿ï¤Ñ¦ÙÑ¡UNASNone@"+ÊW§†ÂLogParabolanone?~èsr¶Ž?"N&ø<C?ïÂ/?Žƒ?"N&ø<C?µ
úåí?Â;ÌÃ×I—?í]þ\€£B?Â;ÌÃ×I—?Ä郕²k?®Ø^:óÆâ?êŹß"e?®Ø^:óÆâ?·ºžÀ؟T?œ1±"Æ–?í¬(hõ?œ1±"Æ–?b¤Ž
˜?fm'&I?ïí[q¯‰Š?fm'&I?™Î_çÇ;?­ÒGìg+?ï1↦?­ÒGìg+?¬Q4þð?¡È¬3}š…?î:ì¾7fQ?¡È¬3}š…?w0÷z¼‡?l#"!C™?ïўàI—?l#"!C™PSR3FGL J1650.3-4600@u<Ãa@O¿îxd•«ÎPÀ7"`X/kþÀ9ÄÉ«?þýøKU¾Î@â¬2#?øwïzÌ¥?Ðs"k(±¿¿àÜù6¦ôæ¿åïólìõ¿ì
ŽDUNASNone@¥…¼£nLogParabolanone?/ˆx'?z?4@KžˆÇ‡?ïþx«s?4@KžˆÇ‡?ª`ñnƒ›?¿|j¿Ò5?îYðé%ŒÆ?¿|j¿Ò5?"q#¼oGç?"¯ûÔV0?ïdvâá?"¯ûÔV0?Áv"ÒÉLK? j\|C!²?ë¢^ËM¬í? j\|C!²?0îU­§Î?+³šëEÒ?ïýâ5Œ W?+³šëEÒ?€ƒ—%€U?ªóXè#•[?ïýñ‡í?ªóXè#•[?w2¾ãt?u4ÿ¸?ïÑÛíÿ?u4ÿ¸?˜ù''µP¯?†Ht4›˜@?ï83n}K?†Ht4›˜@PSR3FGL J1652.8-4351@u[¼w¯d?·‹Y:À8]–
˜à6À:_yv
£W?úÎMÖL¨O@«}ůÞ?Õ	u…ÏI?ïÿî]ýG¿²§3zʯ8¿äòç
2*¿ë¡ ۆ'ÆUNASNone@¡ë•Y³Ð}LogParabolanone?±-'ú"?ÁK¡>(¯¢?íݺM÷¸;?ÁK¡>(¯¢?ֆ
úÙ>d?Í%'»±œp?ä¼ù"`Î?Í%'»±œp?ËËÖá	?±Øs›™~5?é;
 
G¾?±Øs›™~5?Ý!ý˜i[?¸Kg'Ç"?áo3ËxS?¸Kg'Ç"?‰Àõ-](?±Š2ڄ¼?ï˜ü+<ÍC?±Š2ڄ¼?·F]YzÚ7?¿u.O;?í4Tùà	?¿u.O;?¯¡3 PÈé?ªPæºn,W?îìÎpQ?ªPæºn,W?À¬	£EÀ?±)ùr¤
¬?ëÔý»W.?±)ùr¤
¬PSR3FGL J1653.6-0158@0ž=æœo@8ì´Zåÿ¤À8õŽŒöÀ;†"éß,@Gú~¶¿D@þ4x؄?ý'úƒ"I¤¿×'^:â˜Ö¿âFúR
‹P¿å?çx8­¿ïÊ8&¦Ì¢UNASNone@ˆ†–=Ć­LogParabolanone?kª‡B?n͝[^?ïä=Uº¶d?n͝[^?¼¿À¹‡åV?ËÔ²<†K½?ìhèÏU?ËÔ²<†K½?¿‡Côª?ªA\9ée?ìj½}?ªA\9ée?¥ÖÉ5I«?‰æ,hj'?l¦Þ?‰æ,hj'?`"œ£ê?X*יUc?ïïko‡Û?X*יUc?¦>zÐZêÀ?Â2š´Bc?îœRÃW"?Â2š´Bc?¿UØ?™§l¬UÒÓ?ïWœÚ?™§l¬UÒÓ?uå$1匬?b{CttH?ïÔ5·Ðnö?b{CttHPSR3FGL J1654.3-4907@u!ÀD(NÀ°WK@pÀ9»Z´|À:Û¾	»j¥?úp¥+H-@\fA''–@×B¤•K+¿äëÌÂ:øy¿æÓ*ð6ð¿êË×qÿå¿îµN»-UNASNone@ƒSÕßeUÅLogParabolanone	?¬Œß»¬?®ËA«Ñ=?î?§'v¼u?®ËA«Ñ=?®¨XÚ¾?ÀY0âÆv?îzf×>?ÀY0âÆv?ã%1è&çÃ?³$H1?Ùµœ/²0{?³$H1?ƽÔG¦˜í?£Üy•Á?êPŠîYÅ?£Üy•Á?‰æNdMC?"÷Hx1µ?ï›ÐfÆnË?"÷Hx1µ?fþkõ)_?®gXGÍp¢?ï|Èɒ?®gXGÍp¢?ÕÕ´âö.ñ?¶r@‰8÷Ž?å%Ž"èˆ?¶r@‰8÷Ž?'Šhµ\Sú?€Ël²~?"?ïs¬ºU`?€Ël²~?"MIXED3FGL J1702.8-5656@tÆ]cˆe•À"}DUGZÀ8*ºŸ£ŸÀ;'8|HP?ýŒBn@K}u ¾g@ûaŽ»D9¿ßÔâJbyÈ¿å2'¤¬¼¿èSXpj²b¿é®!/>uËUNASNone@~–Ov`LogParabolanone?Äz­ÊB?ÉER–6?êá`9p?ÉER–6?­+aª*e£?ÀO·´rôû?î-Iå&_æ?ÀO·´rôû?åSW'&øV?³J'Øëq±?ÕYPÛ²T?³J'Øëq±?ÂBÀ•˜n? ¸­'šÿ"?ëoOڙû%? ¸­'šÿ"?¤˜š!F$;?©ø¾1?î¶v^"—|?©ø¾1?'xlѤá?­õ~n[X?ït<™I£É?­õ~n[X?Ô©6B»?½C89~Z?å«dÿwÞ£?½C89~Z?Nò%'Ö?±qy*h}?ï}xaQ?±qy*h}MIXED3FGL J1727.7-2637@v}T!ÀD(@FœÒ3>À8–ØÐN,À:¶[Ëر?ýdÕ÷ú@ A]òz@k°ªØ0X¿àëïhò̀¿éýç"fh"¿ï†¾7U#?¿ïø0ðŽjUNASNone@€0Ïþ°t§LogParabolanone?°c 
êø?¿³\ýöª0?íó‹þP}q?¿³\ýöª0?©ÊÒ̖5?À^¨EÈ¥å?îcRÓ6žM?À^¨EÈ¥å?ßÈ7AµØ?µþóӆVD?àätß%?µþóӆVD?·J"=E?˜ÒšÇ5	?í­ %"§?˜ÒšÇ5	?Æ¥ž#…Û?Íaœv²}°?ê{–˜w‰?Íaœv²}°?"ª!L?°Íi¿\-?ïgÇz†¦?°Íi¿\-?Ó´dÊôŸ>?½ èzI¿‰?æ%͚…°a?½ èzI¿‰?}ÕO7€¶Ó?pàDÿÞyø?ïÄUa}ÀÂ?pàDÿÞyøPSR3FGL J1729.7-2408@P÷[ìá@AêÝYÀ8z«°óRsÀ:ÀÒ£¦bÖ?÷¦Zøt"@iÀÆY@8@üÞßHûG¿×Ù^ˬ¿ê…..€`¿ë±N¥®ö¿å·nðèNÍUNASNone@¹÷eýŠÛLogParabolanone?êÚ7¢a?ÌÜ>m+°?Çä—!wÒ}?ÌÜ>m+°?Ò6°kBCF?ÑÐ5b?æä§Ê^Þ]?ÑÐ5b?ê®7¬[´?¬äÒLõnZ?ÅG!OŽ'0?¬äÒLõnZ?àðQÉU?²oóf+V?ßÐ]úmU?²oóf+V?Ýd­Å†Ã?ЕB~Íü?áM©<ž8?ЕB~Íü?¶"RÜ)?ǘ^©?í-uèË?ǘ^©?äG_t¢í?·w¹ ÒÆR?×qAĺ&?·w¹ ÒÆR?¹tý¶';7?ª­?AH?ìÑ`I/¸™?ª­?AHMIXED3FGL J1729.9-0859@.oõHìÙ@+&æS†ÒÀ9Bs9³õÀ;9/bÄw?úþø–T?È@
ÜTÎczÏ@må|ñî¿Øê(@§t¿ì6'üDK¿ïÿ´h¤ž?ïð¦ä/êÔUNASNone@{ÙO
"MLogParabolanone	?á2,á?Ôâ¬"x?ݛ§çÌ=Â?Ôâ¬"x?ç"r'Ôœ?Õ³£ƒÛÊÊ?ÐÙÜWâÉ?Õ³£ƒÛÊÊ?èþêj0?²"´öââó?ÏÄøVW>?²"´öââó?îJ€ÄX"?­z£?ÊÈ?«Wó·ìA¼?­z£?ÊÈ?â
¸]T?Ҕ)Â
ñ?ÛêEWÍò?Ҕ)Â
ñ?Õsãñ›R?ÖÒûªÛ¶J?åF2Vó?ÖÒûªÛ¶J?æ¬^ûÄ?µeæd:¡˜?Ò§CúwÑ?µeæd:¡˜?ãßË'í@?ÓÝα ?Ø@i°%Ê?ÓÝα MIXED3FGL J1730.6-0357@3ͽ@gÏ@/în"ŠzÀ9Ä斢nTÀ;gæ…·?øðMÈà¯@3·«þK?ߣK¥¤¿Ú–ú©T?¶k\€š«N¿â_lµñû¿îT'BÙiUNASNone@™)ó¶E¡ËLogParabolanone?"8ˆ@	ì?¦O.mO‹?ï¯ö™À?¦O.mO‹?¸1VDfÂ?ÄkTHù?ìùÕ7:ºø?ÄkTHù?Êú8‹¦?´mêj÷­'?éA[ñÝ`?´mêj÷­'?ÃÍÏ\?ªà')ñh?ë>¿ùL)?ªà')ñh?€_qˆ?§¢–ž`ªo?テ'…ø?§¢–ž`ªo?eÄ¢SHõ?¶†¬L¼«ž?ïÑÚíe¸?¶†¬L¼«ž?°ÿ[¹eò?¢'­™Ö«H?íý {Ò?¢'­™Ö«H?ŽG—0m7?u)°"&+?ï†á£Ô?u)°"&+PSR3FGL J1734.7-2930@vd*Ã") ?û6«Þ?»ØÀ8•—Œy§À:zŠÊɽN?ù¼Á"Šf @¡œò¿?ö>À?°uñWrb¿åýu·¿ç$ù³yƒh¿å¶$ÿ‹2pUNASNone@žUÍquŽLogParabolanone?ëñ3–QÝæ?Äg¯ÄÔ0?À;1¦¸ˆj?Äg¯ÄÔ0?åí!/òÙH?Îؽ¤ngo?Ô%½ Mo?Îؽ¤ngo?æå¨û%>˜?´;IaLÕ?Ò4®	µ'Ñ?´;IaLÕ?çۇÒ5±,?«g­ž•I+?ÐHð["©?«g­ž•I+?ä õ ï?φOÍ?×À¾ú¾"?φOÍ?Ã¥AX?Ä©]m)µA?민=)ù?Ä©]m)µA?åWñ¢*s?¶ŒÚÓÒ?ÕP»«ý?¶ŒÚÓÒ?Óð<ÓðØp?ºm×£.\¤?æá–"È?ºm×£.\¤MIXED3FGL J1736.0-2701?àWà[õÊ@iÏ!:ã+À8¼°³ ¬À:œ÷½;_R?ù®WÙÛ©	@
1î¯ËŠ-?ùmª*5ˆ£?åËñ»C¸g¿ç¼—šˆNe¿åuµ}"š¿ïÿáïôšUNASNone@"åՁ%LogParabolanone?‰ûûÓ9g?Çy¸?nwN?ë]1¦?Çy¸?nwN?·m»ÏúSÄ?ÆùÉnbo?íH†Em·?ÆùÉnbo?Ø°ì1"?³§ƒ› D~?㧉çtî¿?³§ƒ› D~?Å)ØÒ¥ºö?£Ož_f&?굉ËV'B?£Ož_f&?¹™Ò0†R?ƈÙ¢?ìÌŹï5¿?ƈÙ¢?£'¬œSþÈ?Á¦'WÃò?îÆÕ6C4?Á¦'WÃò?Ò/¹°Kž?¶ç»þ'Ù?æèq£'Ú1?¶ç»þ'Ù?™>Š—õµ?Ž(büÏÌ?ï6ëtF"?Ž(büÏÌPSR3FGL J1736.5-2839@vr÷eýŠÛ?ýn'«?´KÀ8—cW¾,÷À:´²G^?þqõ0K¦@/° ?ò`àëgÿã˜YþyC¿ÛΆXÒ²¿ïÿñÉ 6[?ïöúNKx¶UNASNone@Œö¶y|ÄLogParabolanone?Ƚϯ«)?ËMsjƃ?éйÌ6?ËMsjƃ?ìíq¸²—?Êm'r¼h¯?¸—qÌwÈ?Êm'r¼h¯?߄DO\«õ?µ¢ëÅ
û;?à=ÝØQª?µ¢ëÅ
û;?ïyÔת˜½?'Ñ›8Œ*Ê?Åed¶e?'Ñ›8Œ*Ê?àFła?Ӛè_`žâ?ßrtûï>?Ӛè_`žâ?à—^^óM?Ö^Ùa'.º?ÞÑCËBf?Ö^Ùa'.º?ä½—û‰Ï?´í²}C·5?×"Ðìc?´í²}C·5?雝yðS\?Íz©XBP ?ɑŠ>²?Íz©XBP MIXED3FGL J1737.9-2511@B¡µÇ͊@~HÀc1þÀ8O#—´½À:ÙXÌIð?ý
Ä<°`@ªNò]U@ÔäÁ5>ü¿áð²Q˜Æ¿é8¢=­	¹¿ì5Ì>ïÿ>"Ó—uUNASNone@‡¸þùÛ"ÑLogParabolanone?Ëkr"öéÆ?Ð˔¾h†?é%#wBE?Ð˔¾h†?¸íÔÈV?ƅ˜h0?ìâE}ô³­?ƅ˜h0?ámEÿ\0?·}ê";™?Ý%tÉG¡?·}ê";™?ÊL1ÖU¦i?¦ß%ŸÕQ?élóŠj–f?¦ß%ŸÕQ?Å
ãB…
Á?ǎíóQàŒ?꼇/^½P?ǎíóQàŒ?¤ÎᎠ£?Àÿ>F<?î¾cµ?Àÿ>F<?Õ­BHúµ?»<íŠ÷.?å)^ñۂ¦?»<íŠ÷.?Ÿ`L1aü?ˆ×FÀ‡-×?ïýžYzx?ˆ×FÀ‡-×MIXED3FGL J1740.5-2843@vy>Õ(?ñVWûi˜À7kŽ#CÑçÀ9Ó=¶CôL?ùIA<‹@³¼Òì™@ir©´¿Ï…Xþ㏠¿ç»³Ï½¼¿é|ç´Q"T¿ènÜ*ÝUNASNone@Š8½Ùb·LogParabolanone?´õ7:‰&?½>
#K€ÿ?ía\¹
ðk?½>
#K€ÿ?µ€çZ½qØ?Á5I
2?íOãŒÔå?Á5I
2?Ó(Ò¦Df¦?³ÖñÜj½?æk–¬ÝÌ­?³ÖñÜj½?Ђ›?©5
àÅp?ç¾²vùö??©5
àÅp?Í¿Hy?—€q|w?ïˆÉáÙF?—€q|w?—zˆó‰C?²™9úpÌ?ïD+¸Œñ7?²™9úpÌ?Ó`n™€?¶Tck'«?æwvÏȳ@?¶Tck'«? í/²Ž÷Ä?W:ór³9?îñ-×"?W:ór³9PSR3FGL J1740.5-2726?妟ê$Ì?û»èÿ2z§À7ù/‡­À:3µ«HÇ?ý§7è¥@1	½@ÛçF÷¿Ùv.ü¨î²¿è{+½ÑÞ¿ê'ôRLÔ¿ïÿ›o÷M™UNASNone@†!P©*0LogParabolanone?–ýFÝÍ	º?°€·=¡ÿ¢?ïHÉH'r?°€·=¡ÿ¢?°Ï÷-+Xà?Ä7rh.?íævÄ?Ä7rh.?Ñ6Q3,ô?²~jœ´‰¾?çd×fiý†?²~jœ´‰¾?²¾²˜± Ñ?"'¤»]O?í¨)¬÷šV?"'¤»]O?±œ.†f'#?…N±q…?íÌz/Nª¼?…N±q…?›Ý˜äøCœ?½n4ċh\?ï!8Ês?½n4ċh\?Îg£Žv6#?´RLj×?èfbrw?´RLj×?~Ì®Éöfv?gŸ»æÛIÈ?ïÂf¢©ì+?gŸ»æÛIÈPSR3FGL J1740.5-2642?ôÞ i—sO@û¿¼CÎÀ8ÏËRyI˜À:µ½Ñb^?øºQO}ì•@ìG'd?ô4đ?¿±ïGºU†,¿àìi9i¿æIæ¯æ¦×¿ïe­¾ê‹úUNASNone@˜WLL˜_LogParabolanone?X÷°cå¢?mg6?Ä
?ïó"|Q	]?mg6?Ä
?´úõÏÜhú?ÅKs2&Ä?í`¡Eèö?ÅKs2&Ä?ÊøŸA+÷Þ?®âe{´ö$?éAØ/µ?®âe{´ö$?Áä§rRáW?¢_ò~Ä?ë†Ö#kGª?¢_ò~Ä?Ob`ºƒ]¾?`¼^ÐMëZ?ïø'h§¼?`¼^ÐMëZ?Ÿî&Oj?¾oªaµI?ïn¿È¥?¾oªaµI?¿i7«VÊ+?¯"œZ@û?ìÙ
•&»?¯"œZ@û?Œ±"ýOp?vŠƒÑ¯(X?ï;tA½²?vŠƒÑ¯(XPSR3FGL J1742.6-3321@v>p†nD¿üdóºw_³À8)+hc–¨À:wfÀ(yœ@kä'fI‹@˜?&†}?öñ ԋÝï?ËÄÇ>\Jó¿á†ÿI\ül¿êôϺÜ¿íô[L
lUNASNone@'à;çl‹DLogParabolanone?Aäó$_×*?MedŒ0JW?ïû†ÃD?MedŒ0JW?¤ï'ó²ê£?¿–I1fR?î±àÄÑV?¿–I1fR?¦ö•Âü<È?žóñqf?£ùwƒ?žóñqf?¨o®í?‹³ûÌgí½?î¹.H?‹³ûÌgí½?Gž¿mp A?T¡
«
?ïúOà›"?T¡
«
?Œeé7p-?«¥Šòðtˆ?ïŽh[9_?«¥Šòðtˆ?Ž ÌÛé´à?•/sù–Á?ï…|ÌY_m?•/sù–Á?tÌ@Zm?fu§ÜÖ?ï×ügˆê?fu§ÜÖPSR3FGL J1744.1-7619@sѬ<žìÀÀ6x›ÇqC9À8"{?;2À;]"mé§@W±\®×™@'p\"y?ó¼†=Ç5ß?të¸cËäÀ¿Ù&t;™½¿åÉâܦ'¿ïÿíkÜOªUNASNone@Žb¸}¿HLogParabolanone?X½vž¯?dêvT:×Ò?ïó¡DÞ¬H?dêvT:×Ò?®×á™[²ã?ÂI¤·×X?îæ…Á²?ÂI¤·×X?¨Þ!Ë>"?@*xµ°?îrã&Ç?@*xµ°?XcÐQ?!?uMª;Sk?pÌys?uMª;Sk?d­]ÕÍï8?rÁ"§yF?ïëR¢ôA?rÁ"§yF?çû#ϐ?¶`Îêá…?ïÀ&̤?¶`Îêá…?'Õ²Ãnü£?f¨Ì)ž?ïiRj
Ãk?f¨Ì)ž?\@e%Ÿ¨?Q7 ‰R›¤?ïñßÀ3P(?Q7 ‰R›¤PSR3FGL J1744.7-2252@N8C=lr@
©‹XߕÀ8¢Á¾{Ñ2À:Ò('fvW?ý 'b"s@^ߥ—~·@÷§üÞ¸]?¸Ø>Óp¿ìZV1ò¿çRg!]ƒû¿ïÿ'Õ/FêUNASNone@I;â.]áLogParabolanone?²cNvØ?¾`¬×ÓªÑ?í½SŸ±®?¾`¬×ÓªÑ?¬"z°l¼8?Áüøá[?î7¸U=ìl?Áüøá[?يÝ9è•;?³ÛÈ Ë?ã:'cµb?³ÛÈ Ë?Àõ+yw?Ÿé©n§<??ëþBµ !¢?Ÿé©n§<??´ªâBÿ?¼ßø×i°?íj£·Õ™Ð?¼ßø×i°?™‹ì²Æ;c?¹Ðn#ìe¼?ï3 š%õ?¹Ðn#ìe¼?Õ%À«£©µ?¹\øý¢ñ?åmª.+%?¹\øý¢ñ?"§—ýðر?€…¾‹Ž?ïZÃ@9´Š?€…¾‹ŽPSR3FGL J1745.3-2903c@v}Ò½<6¿"" 
êÀ60•âTôÀ8¥ãÛÝ@%{‡ŠÎP@	ùù€´ñ?ô¡9óÁ®?æÚcY\ë¿à'î}î垿ç–Ûñz¿ìk]ãyÑAUNASNone@ž=‡+JLogParabolanonep?5Ĕ›qáW?<e!aBÎ?ïýGm@¹ó?<e!aBÎ?¤ ‰GÈß?ÀPL_¡s?î¾5÷¢}2?ÀPL_¡s?"wftñG?"¤à¤¹ëñ?ï{dD£&?"¤à¤¹ëñ?tÙ
ۇf?bb-Š
rÍ?ïÖMä†Ê+?bb-Š
rÍ?;ŽÛ¸"l?A"ÆX/†?ïüŽ<T€F?A"ÆX/†?ŽE,#?¬7†§j
â?Ý'?¬7†§j
â?M6WZ#?˜;ÝYjˆ?ï'Ê]œW?˜;ÝYjˆ?RdÞ·?K]sÆã!?ïö͐°Ö'?K]sÆã!PSR3FGL J1747.0-2828?áÔG '¨;¿¥(ÚûÊÍTÀ6¦¤Gr…YÀ9Æé]ý@úÁC`Ó@ÂÁ†º?ûtS5G¿Ä34	òÈ	¿äÅHEWç·¿è]xãQÛ¿î"ËÝUNASNone@‡1Ùb¶®LogParabolanoneP?ÉÆà(
)"?Ì<Vّ½h?éŽGõüµ·?Ì<Vّ½h?­
‰{û?į½€"?î/'nó—?į½€"?Â6p°ÓX=?­'øü°´ ?ërcÓË)ñ?­'øü°´ ?ªl}B%?'à>¯î8»?î_™2?'à>¯î8»?ÓS0Pw35?Ñ©½¡"Bu?æVg×Äff?Ñ©½¡"Bu?˜X?àŠ8?½=ÿ¦$'¹?ï=>6þ?½=ÿ¦$'¹?Ù]˜VÎmâ?À"0PÕ°?ãQ3ԘÉ?À"0PÕ°?Œw¬êOF?ˆÇ»þ
?ïŽ!L<)ã?ˆÇ»þ
PSR3FGL J1748.3-2815c?ìà³3ž"¿Å#rö"À7âÃ2ðUÀ:h)qéQh?ÿ'´µÔ¸©@9›
²ái¿þÞ²G»U?åiáypô?ƒ4K´ýÙп͝D¬q&¿ê"ªúƒÙUNASNone@¯î°£×
=LogParabolanone$?ÀH%©ˆ?Ï¡h»*c?ëÿíþö•ž?Ï¡h»*c?½fÍ1?Éï=m§Uø?ì_S&\z?Éï=m§Uø?ÈqõG·œ?¯nV|s?éギÿ?¯nV|s?¸'¿N)Ʋ?°ø¢Ó$
é?ìíÈH…š?°ø¢Ó$
é?ÉlÀ³	Ù?֍D?ä¶<?é¤ÏÓ<}Š?֍D?ä¶<?¦£'Ø`I"?Á㕛Þx?î•ÇÒ^~ˆ?Á㕛Þx?Ówþ'/B?µXåmSµ?æD¾ýè_?µXåmSµ?"4r«÷¹? ìÉ?Å)û?ï^\j C? ìÉ?Å)ûPSR3FGL J1749.2-2911?ȦÃ"Ôì+¿êתv`¯À7Í«û›í1À9®"ñ¹ì?þÐâ»Ìtb@
ۼܿ´?õ$ýÍð
?ïíßvȉF¿Üن±+þÙ¿çLÞ±ëcÖ¿êÅùé‡åßUNASNone@ŸüH˒LogParabolanoneD?!t™4ÖM"?3t¨®=u@?ïþè¶7_?3t¨®=u@?±²ˆŠÊì?Ĕx#
‡c?íɮ}?Ĕx#
‡c?±"áUÉIÛ?£nÎYˆÀ*?íÍcÕ+Yå?£nÎYˆÀ*?½è=ãÝ­? ÆñVI?ì^âøC"J? ÆñVI?m=ºþ±?"Âe¦ß
¨?ïâÂE<þ—?"Âe¦ß
¨?šwtë4M?½+…Œ=ÝÓ?ï,DXÁÚx?½+…Œ=ÝÓ?¸]©Ð½U?¬æ~×Nðy?ìô]Êáe5?¬æ~×Nðy?—^ô°€5Ñ?…ÑØèH…(?ïEZ—{1?…ÑØèH…(PSR3FGL J1749.6-3133@vcpâÁ*ØÀ×)9µ-tÀ8²²eByøÀ:u'OÐ!ì?úHDºšH@
ÒòÖ¡¸?û|½›+•¿ßäk•ádp¿æîrÇÑC¿æŸPµ¥ô¿ïÿƓðÖUNASNone@§³Ð|…LogParabolanone?édÐfà3Ý?ÌB6äÌ&?Êl¾d0?ÌB6äÌ&?Ôu8F'l?ÊÊð¡	ÇÌ?åÅcÜô7J?ÊÊð¡	ÇÌ?âÈðȐ¹1?µÜ:h¸y?Únnލ?µÜ:h¸y?àÂoˆ›fñ?±ä´êRÐ¥?Þ{ îÉ2?±ä´êRÐ¥?Ôò÷ÕuN?Ðß\Žm¸ã?冄EXò?Ðß\Žm¸ã?¦ö,Kö>.?´u'µ«¼ê?;\ý?´u'µ«¼ê?Ø{Fzì8?¸ü0.õJ•?ãùÂ\‰ä?¸ü0.õJ•?Áëåtl1?®ÞÚv›¢9?ë…¢äút?®ÞÚv›¢9MIXED3FGL J1753.6-4447@u±]ÌcñAÀ"Õ5†Ê‰üÀ9dßý+9jÀ;cìƒKy?öPrß­*@
·²ˆÓÏ?÷Y˜1å€M¿Ùl°f:¿Û¹Š¹	ª¿äT*\¨€¿î·(ðmUNASNone@œƒp ě¦LogParabolanone?¸e²mmD?–
úw?ï‰iD»?–
úw?ÁhCs¥Ç®?Ãy
‰ò?ë¥ï#Ž?Ãy
‰ò?×~øËz´ž?´pÍêh9?ä@ƒšB¥±?´pÍêh9?ԊÓN'UA?«¦nÓÃ?庖X¾Õ`?«¦nÓÃ?d™ÎąíÌ?nýµ39O?ïëf1|º?nýµ39O?™¢É¹´ü?²"?ã[?ï7¢é¤sè?²"?ã[?²ÌBñé¨*?¥§ÚÅ?í¦w¡ÞGÛ?¥§ÚÅ?£UJø0Y¸?·Ë²K?îÊ«Pa}…?·Ë²KPSR3FGL J1754.0-2930?ÜÖ¦ YŸ¿ýÊÌ&´Ÿ¯À7çå7&ݺÀ:2ËÏvË8?þ_¿c×ñ@[çÿ@G$êp Ï¿áÎ*2-¤©¿æ¸€"åÕ²¿ëÁþ¸,VË¿ïü»8¿}ôUNASNone@lAž0PLogParabolanone?|Z69Ž?˜A$(!ˆñ?ïÇÏJç–
?˜A$(!ˆñ?²RQ¶1þö?ļFnñœ²?íµµÉG~'?ļFnñœ²?сò¥ñ¹
?´eiºy{&?ç?­#z?´eiºy{&?ÀªòÔÀ®?Ÿý¿@Ĭ?ëøUCJÏÔ?Ÿý¿@Ĭ?¢´y:pŸ?·•·Ç;½?îÔ¸lK5f?·•·Ç;½?™#%¸»É?½·ÉÛUљ?ï6æÒ:'¢?½·ÉÛUљ?ÍÁCgïä?µ$AĬ¨ü?華&Ü?µ$AĬ¨ü?'PñÒCBñ?|:hdKË?ïuxqDª™?|:hdKËPSR3FGL J1754.0-2538@?§ëkôE?µ»Ä¼²ù<À7æyó$÷À:T9ܚ *@wp×ÙpI@ÏôTüÊ?æގ¿‡%4?ïÿ¸$B`¿ÑRôþˆöM¿âaåí"¿ë#‹²(›UNASNone@¥N$oiLogParabolanone?®h¼qhÇ?À¹wÂã?ît?dfS?À¹wÂã?³záƒÏ>?¦OÏ9þB?íœÐ£Ï†?¦OÏ9þB?¾BÆÛél¸?ª'»´5L?ì7§$'Òi?ª'»´5L?ÇÊw€™?ªl‰/Ýöè?ê
b>8ŸÚ?ªl‰/Ýöè?Æ°ÖÂDÂ?ϕù=»nÎ?êSÊOnþ?ϕù=»nÎ?£(n÷#G?¼ùS[¥JÛ?îÍysPì?¼ùS[¥JÛ?½)ŒÍ??±I1¥©G?ìZßN|X?±I1¥©G?­#æ0˜pœ?›Ai†ö6¥?î-Áœöxö?›Ai†ö6¥PSR3FGL J1757.7-6030@tÐ,<žìÀÀ1*$š<À:W"'iÑUÀ<;¶N?÷6&:&l{@{QZÀè¿óñF×Tæ?jiЬ<øÇ?ßÏ|k¾¿Ï	K®)I¿ë¹KÕZSÍUNASNone@¦µ¸Ôýó¶LogParabolanone?â^$ɖ•?×Úg¥*ÇT?ÛC¶lÒÕê?×Úg¥*ÇT?ç¯{ƒ.J?Ñ]Y/yÈÌ?Сù£Åm?Ñ]Y/yÈÌ?߉êJÈ6v?¸Î¿þù"×?à;
ڛäÅ?¸Î¿þù"×?âøҚNÜ?ÃÀãÄyÛÓ?ÚtðËbG?ÃÀãÄyÛÓ?Ó©àÆv=ì?Ù¯XÙÇ?æ+œÄá
?Ù¯XÙÇ?ÒôG2¦?ÒÖ^êI?æ…Ü?}æ­?ÒÖ^êI?ÕJ'(?¶åÜŽà?åqZ¶¸kõ?¶åÜŽà?É\×w˜?‰Xï/x>?é¨û¾Ê"?‰Xï/x>MIXED3FGL J1800.8-2402@ÓW>«6z¿ÜíWœI!\À7VIÿ''ìÀ9¶0©ë÷?ûepÈ@½ÉljÁà?ù1%'¿Ò
'ús¿ãÈÓÉ@PR¿á_)oÁë¿èᏄ—ÔÈUNASNone@¬l(õ\LogParabolanone?£g÷`MÉ?°ð(T¾æ?îɀ‰þ#?°ð(T¾æ?µ^‡RwÐ?ÁZö>œY?í_t/Zi6?ÁZö>œY?ӆ¥ò©'?´Œ}ûó?æ<ü­«7?´Œ}ûó?Ò%œ¦X2¶?«¿f8;?æí1¬Óæ¥?«¿f8;?rŸ7;ù#ò?z¹¿æGº¯?ïÚÁ'§ª ?z¹¿æGº¯?•nd8n}?±ÕÁ,ØK?ïTŒÞ•|?±ÕÁ,ØK?Ð=Õ õ?µƒµ­{—´?çá|•/…1?µƒµ­{—´?°¹­"°ù?""ç	+PO?íèÊM…]¼?""ç	+POPSR3FGL J1808.3-3357@v`÷<ÉÀÚ\¢˜EÝÀ9w;ØbçÀ;DŸqIï7?ø
.j€@oÅz¤6?ôž9ŒÈZ¿Ö¾l$žù^¿Û‹ÿÅ*¿çVïó9ëV¿î°¸ë!)NUNASNone@•¢Â©"áLogParabolanone?ªч!?°È§\–õ?î^Ÿ2¾KÞ?°È§\–õ?ËK!7CtZ?ÆLÜ|˜,?é-7²/"é?ÆLÜ|˜,?ÔÌä¨>U¯?´¤Hº¨	?噍«àÕ)?´¤Hº¨	?ÙTeÖQ8Š?±fi%?ãUÍ×c»?±fi%?~ñ›¥˜Är?Š×ÎsÅû?ïÂÈÁ-?Š×ÎsÅû?›ä¨æ²‰Ò?°B<Ð}ÌÙ?ï Ú¸ó§?°B<Ð}ÌÙ?²jê¯ÕÍ?¤#êé3?í²¢ª†Ö?¤#êé3?¬¾ñWpª7?››éZ@ ?î4êÍ­Œ?››éZ@ PSR3FGL J1813.6-1148@2OµIùH@³Œ|z¤âÀ7ÁÐ\¤EÅÀ:¾­OY?ÿ"VÔxß@¤[©ôۊ@¸½ÄMc¿ÝˆZá'Ĩ¿í7úb˜b¿å
V<-E¿ïÿYƒ÷=[UNASNone@}ÛçB™Ø"LogParabolanone	??+ÚTJ|?Pë9
V™"?ïü‡?Pë9
V™"?šñ'«ïÇ?¶xÿ´']{?ï(sê»þ§?¶xÿ´']{?΃ï+z	å?±-,£<ª?è_5!}‡?±-,£<ª?"Åtí&"Z?€ÕÊüë?ïaÔX²H½?€ÕÊüë?~úò«'éX?p&=2cË?ïÂ
ØjÝ?p&=2cË?€ÊŽ½0Š?¢[tUHy?ï¼ÕÇ®f?¢[tUHy?͉әּv?¸0Uë~o›?蝋ŠPã?¸0Uë~o›?e¼oaS®[?\O¸Üù=`?ïêC×é?\O¸Üù=`PSR3FGL J1823.2-1339@1š¥ç…µ·¿¸€,5=$À7jf¦'GÀ9R[Æ?ùJšèùÿ
@䓳%±À?ýwã:"¿Ø`ð"¶—¿à¿Ÿ×eü¿ä5†‡8¿è"†¸ýsDUNASNone@™?!aä÷fLogParabolanone?©ÄÖlva?µzóÅ)ØP?îc²™¾Ú?µzóÅ)ØP?±ë۞¶^Ø?º¿™¯$Vˆ?í"Œ
·E?º¿™¯$Vˆ?Óͽ¼ÓIW?µ
"?æ!!–[T?µ
"?Ô>Þq(Ðó?ªjd!¡?åàÇk—†?ªjd!¡?€TI,À"?‰ùJW‡¾?ᆴێöA?‰ùJW‡¾?SϟŠÖP?¦,!s§žh?ï}a'Úmþ?¦,!s§žh?Ñ1(E»Ã?µÕUæÊ ‹?çg~ëÝ"?µÕUæÊ ‹?±zÊIÛ?"ÌÐ&R?íÜ_0´u5?"ÌÐ&RPSR3FGL J1827.3-1446@1ud0+A¿÷½¢!þW‰À8ˆÿI ÛÀ:•ýʛš%?ö'Ò€@
'Ü®—,­¿ía'ÞÒo	?çtÝ̃¿Ï(œA8ž¿ßH–3€¿í³rB_ŠUNASNone@¥ZÖ_Ø­¬LogParabolanone?ÛYLWÖ?ØR'†u?âS?YÔ?ØR'†u?ÚÖÝëœà?Ó¥êKtí?â"ò'
1?Ó¥êKtí?Ò¥8_—ë?²Ò?v!?L?æ­1cÐ4
?²Ò?v!?L?ÜUëÇYþ?Â8…œPq÷?áÕ
}S?Â8…œPq÷?ÂóSt?ÓÜE·U}q?ëC8ë?9ã?ÓÜE·U}q?Á4A#ˆü?Ê¥bÝgF-?ë²ï·;Á?Ê¥bÝgF-?¼w>ÐË4?¬kM±ÍÝ?ìq%æ™}?¬kM±ÍÝ?¸ýápŸ"¨?µ•dçÇ?ìàCÑÞPû?µ•dçÇPSR3FGL J1831.6-6503@tŸ?¼À6gø"»ì«À:‹†³
&À<e»À5Ö?øð+oð@"˜ýgtX¿õÇlãË¿å뒙0yV?Á•î¿:èß¿à8ƒÝ£<¿í…̘IhUNASNone@¤Šœ¬1'LogParabolanone?Úú)­´"Ù?Ù{ãõhÍ?â'ë)%µ"?Ù{ãõhÍ?ÝÀÐS®Â?ÔS³²¹??á—Ö(ž¸?ÔS³²¹??ۉ zž×œ?¹¿DRY-?â;o°"2?¹¿DRY-?Ô&_ƒPàv?ÂÓêßmŸ|?åìÐ>WÅ?ÂÓêßmŸ|?ââ0xmÐ?Ú#?[pÐ?Ú;ϟ$`?Ú#?[pÐ?·'ÐT¾3²?ÅZ2=6c·?í
¥õ>þ:?ÅZ2=6c·?ÕïìCb?º¾ºßè?å|	õÞO?º¾ºßè?¡ŽzB˜%?¨(
вmM?îç[§¬¾?¨(
вmMMIXED3FGL J1831.7-0230@<u^á6ç@	Ó˜K$ÂÀ7àùx&'KÀ9ÆõkQ‡²?öÉLÌKž@»PÒ@´þh{>¿ç"=ý;ª{¿èóAç½$¿êF$mƒÍ;¿èõM¤E£UNASNone@Ô1²•êLogParabolanone?†$‰HÔà?ªo`â£6?ï§ÏmÍ=?ªo`â£6?®/šBÿš?½a~ª?î[ÂQ&?½a~ª?ÐÚ1GSYL?´IïÚ¯O?ç'ç\VSZ?´IïÚ¯O?Íâ‹›ee?ªŽ¾ƒº³e?è‡]8Y&§?ªŽ¾ƒº³e?p<òbRA?'Á'Ô¡¦…?ï߆sµ?'Á'Ô¡¦…?üc'CV?«]'°&¬p?ï€q÷'ó?«]'°&¬p?Ì»ž!5&?³‰ð`ÿ?èÑ>Xw²¶?³‰ð`ÿ?šÄ4LL?ˆÍt^îð0?ï/YÞ(ûÞ?ˆÍt^îð0PSR3FGL J1839.3-0552@:S¹EÅ¿‰ÕÓ0¿ À7±EˆÀ9SÓ[\G)@cªpCµ@ûÊ"x{?ù"ü(¯÷¿´Æì`@&¿Û̕asû¿ä徸âà
¿êës§¨·*UNASNone@£('䎊rLogParabolanone?†›š_.?fúb÷kÆ?ïÿ[Ëñr?fúb÷kÆ?–‰Ñ(ä[?´†cGRBü?ïK±vÚý½?´†cGRBü?¨ã6»? ´…)n?îŽîšÒÕ? ´…)n?›´JŒû'k?€óðF‰Z<?ï"]«Še}?€óðF‰Z<?(·!ª‡R¬?!À¬ËY'?ïþtŽÐ?!À¬ËY'?x§'U«²?ž
o8ÎÑÕ?ïΰÜΙù?ž
o8ÎÑÕ?~¬8ãb?›.C..?ïÃʧzû?›.C..?qò¬¯D×n?_ý\¸ðÓ?ïܦ°"™?_ý\¸ðÓPSR3FGL J1843.0-0359c@<mCx$Õ?¦µ¯`À86(ï'µÀ9Éh%ƒGH?÷Çy8¦È@š#WH?õÑÄ ÙSï?ÛÁòu¿Ý˜˜ÊLü¿äh˜pàÎó¿ïÿÕÄčUNASNone@£™Àƒn˜LogParabolanone1?ŒN6ÍO1I?õ8¬A?ïŽÇ%{j?õ8¬A?Ñ
3œÜço?ɳZµÙ[?çzæ1'ŒI?ɳZµÙ[?Ç	ï³EV?®xÍNÛbð?ê=";Ó.ª?®xÍNÛbð?á;I‹tE?°û…¾Ð­?݉lÄéu?°û…¾Ð­?|œ×Zp?¥AnÉÝW?ïÆÇȉ¤¸?¥AnÉÝW?³¢Šøϱš?¹Rÿ1à$?틮¡†­?¹Rÿ1à$?«<ØB^ºÅ? ×ƒ¥Š•O?îL2{°Ù? ×ƒ¥Š•O?ÈèceCëV?­ó™*¹(?éÅç&¯*?­ó™*¹(MIXED3FGL J1843.7-0322@=çáüú?ƍ¥šƒÏXÀ7ªñÀ9À¨á59ž@"Ùz/F@'Ý<Ü@CÕÖᣟ¿Ü;š<#>¿çòµ0Æ=ß¿êmIçՑ¿ïÿAHl"UNASNone@ÙÁü2LogParabolanone?¥›èVm?±ÏgbK	û?î¯6P÷y?±ÏgbK	û?–µçíŠi?¶H¤õÈb"?ïJP—X]?¶H¤õÈb"?Î KmfŒ?²H<<¶?èwí$¹¦]?²H<<¶?µƒÆ¤̧?–—±«ìÔë?íO‡+¥A»?–—±«ìÔë?¬ÿ¸4ðª?¸­5ZdVj?î0|ç\E?¸­5ZdVj?ƒÝ´¼·K?§w±'è~ä?ﰉ-ÌÓ?§w±'è~ä?Рºty­?µž}š°Q?篢ÅðÃ*?µž}š°Q?GGšÑۈ?{Z^oõÏÜ?ïŠâáPb?{Z^oõÏÜPSR3FGL J1844.3-0344@<˹M"¿ÂŒæÃCBÀ8I­Ï±ƒ›À:9ºHf?ûîÍÕý£@j#²Œ¯¦¿Û´ÆVø?ï÷sB܍N?Èé"}m¿á_ûÎBÓ¿ìtĚúÝUNASNone@©ú¬1LogParabolanone?Êö¸ä7¢"?Òaˆ(¶‹ ?éBQÆò_?Òaˆ(¶‹ ?¾Ñ~ÉoÜB?Ã@ô/ü‰?ì%Ð&Òx?Ã@ô/ü‰?½=\ŽÃŸ?«?´ö)?ìXTn'Œ?«?´ö)?Й^;Û´'?¶öZ×}Z?ç³Pâ%¿?¶öZ×}Z?¿Ëþ¹·yÝ?Ñy5¿Dö?ì€(ÉÄ?Ñy5¿Dö?¨YPM?·ñVn÷"†?îºk(öw?·ñVn÷"†?¬ª‹¬'-?§–gštß?î5^|7M?§–gštß?°v׫êÊ?¦ƒm­
?íñ%
•I?¦ƒm­
PSR3FGL J1848.4-0141@?…fîW¿¼Öpd—gÀ6ã¸WÊÂ1À9‹‡Öùvy@¥cSa|@´Üú‰?ÿSqç£è¨¿ÔàÜJ»‡¿çÈPó¿æv×·%_z¿î"Í]UNASNone@•\×ÛôˆLogParabolanone?\¬qñà†¬?i©´Oð†¥?ïñ©ÇJh?i©´Oð†¥?˜ÙK‹/1?µÜõÈ]‰?ï95§ñdö?µÜõÈ]‰?¡w´?¬úøS?@}?ëz}ú×¢?¬úøS?@}?—ðC–½"?Qzʸ&Î?ï@eՋ§?Qzʸ&Î?rBdd?{5ñœ"&?ïÛéÓBÝ ?{5ñœ"&?Slá3b?§oN[F'y?ﺲL²¤ò?§oN[F'y?ÅCá%?´7JS$.!?ê¯8¿x7?´7JS$.!?q¾Ø(¸?a¨s"(óà?ïÝЃ÷­?a¨s"(óàPSR3FGL J1848.6+3232@O$¡œZ@-| fèlÀ8ãÌґÀ:]vfœí?üÑÂèbÒ@{þÔü?þçÛv]ÕH¿¤\¸råµ-¿éôsH»Ê¿å¸±Òø¿ïŸaæ`,øUNASNone@'¥t9XbLogParabolanoneP?ïE`Q¤bu?§ó;1À}š?—SõÔ
·G?§ó;1À}š?îÖÑ®'€ú?´†=#'zm?¢'åçða?´†=#'zm?ånI"¢†?³åº7&?Õá#mººô?³åº7&?îñF©²–?"f028;¥?¯Ðë•d֙?"f028;¥?îža^-¡"?¥ßÒh6-
?¦ê%æÖ?¥ßÒh6-
?ëÁ»èŠ(Ê?Æ®¥G͟?Àù]×\Ú?Æ®¥G͟?é\{t?±ŠKz=8?ʎŠ/Þ?±ŠKz=8?ëè#Ý|•?¯:IHŚ?À_sðŠ
­?¯:IHŚAGN3FGL J1851.2+0423@Bh"pdìê@d}€^_1À8'­K'E¿À:T\Rn?øè뗾"@1+¼ÇF@šO'ã—¿¿ãŨM!Ø¿ëÄ7Da¿éF	Ï*N¿ïÿÚLÅ´UNASNone@{.\ú¬ÙèLogParabolanone?¸ï
Èo•Æ?Àŀ°ú?ìâ§H—?Àŀ°ú?ªÆ¸¹)ß?½Z²‰0Û?îS"t–ªÒ?½Z²‰0Û?Ý·'9øìˆ?¶=9gòÛê?á$>㉼?¶=9gòÛê?Ìžl€öy?©/
^¸?èûXdßÂb?©/
^¸?¤ò-YU?µ7ãp»•?î¸ßâš?µ7ãp»•?"6OÕí½?±T«ËAÔ®?ï^MƒŸ?±T«ËAÔ®?СÁ"Ð÷?½^$Ò·^?ç¯n—…?½^$Ò·^?¡'æ$Áé5?ó‰?¨c?î큝Ï^M?ó‰?¨cPSR3FGL J1857.2+0059@A<YÈÉ2¿êçLàƒböÀ7À!)Es¨À9wúÊ6˜?úSÀý
Ø @.…fîW?õRtK×Cô¿àû[4û¿ß£†ŸcT†¿áNnokÀ¿éE1çwcUNASNone@¨(¾vÈ´9LogParabolanone?"9ޜMÁ?¥ØÿKN?ï^1ӈ?¥ØÿKN?Ø%Ɋšp?ÐS"ƒÕ."?ãöí:²È?ÐS"ƒÕ."?Ñ6^‹H?³åØpÏw?çdüк[ö?³åØpÏw?ãðå6꼑?²3`¹˜?Ø5'*†ß?²3`¹˜?e9Âp1Ô)?m{¿.ú¢r?ïêÆ=ͧ$?m{¿.ú¢r?·º‡?*áv?À"SÀ'¢Ã?í¯(bA?À"SÀ'¢Ã?Å®±‹0?·" Æ´"×?ê¹ÔS˜4?·" Æ´"×?Ò1¶[q?Þ?µ‰ÕûKo¨?æç$ÒG`?µ‰ÕûKo¨MIXED3FGL J1857.9+0355@B•Î|Ð57?Õñ÷(ÀéjÀ87¸Óñ"À9Ü7i"ÙI?ûMFˆï@Cˆ?ÿõ?úÆ3
nmò?ïšÞw3#¿á•¿Ù8/¿êºÜÓç.‰¿è"HÒõ UNASNone@šy¥`A‰7LogParabolanone?ª"(jAà?¹èX¯?î]Ý~©[â?¹èX¯?À¨…‹«Ön?Ã9׌eÌ?ëÕޝ
d?Ã9׌eÌ?ьy	Ô?´<yá*â?ç9Ã{rð–?´<yá*â?ÙÖZh	m?²hRFŽ?ãÒËû|Ê?²hRFŽ?lfDãÍÛ?x'Ìü¡ì?ïãæ™ÒyŠ?x'Ìü¡ì?¤•53xp?±p;œŽ@ ?¬ñ»?±p;œŽ@ ?Éò5–S­Á?µi1%·º?éƒršk?µi1%·º?½zïaÕ?«Žbâ"t?ìP¯ÂÐ?«Žbâ"tPSR3FGL J1857.9+0210@AÍÄupÅ¿ÝyO܌À7iKB±ÂÀ9³ŸAyG?ý­åSViC@dõOÍÈ ?þ=Ž@u"¿äf©#Ǩ¿ã3"]¼¸q¿æ÷ègï
Ñ¿ìÕZ›¾CUNASNone@õè§æ›LogParabolanone?S	=ÆÖñ?er7XÈuP?ïö{aA°Ç?er7XÈuP?£í, "W?º§ÐWà€?îÁ-6;r¿?º§ÐWà€?º~Ïål<%?§Ø+°Êó
?ì°&Rx{?§Ø+°Êó
?Áòð7‹¯? ;¦8Žg?ëƒCò>T? ;¦8Žg?<—Þjê?4ùÙ¥ù>?ïü
ëê¹?4ùÙ¥ù>?†žJ''??¥³¥ÃÐM+?牢×õõ»?¥³¥ÃÐM+?Ÿ†#ÓÁI?˜ÜUѧ?ïÎáFxØ?˜ÜUѧ?–÷ýཅâ?€lr`ñå'?ïH@#O!?€lr`ñå'PSR3FGL J1859.6+0102@AeUÅ.rÚ¿õ¶âdä†'À8
šôãlLÀ9ј:ôÉ?÷i§¡D2à@éüíÑÕ?ÿ'%Ÿ í? I^Ó&¿ãoòÿïíl¿æJÀŒ¼UJ¿îŸØ"UNASNone@4H˒:LogParabolanone?¦[v‰c©?³BIþ0/
?îšHž²æ¥?³BIþ0/
?Þf`=?ÎgÐ$V\¿?àÌÏýar¿?ÎgÐ$V\¿?ÒÝW@•?±Ë`M3È?æð'tÔ_¶?±Ë`M3È?æº%2òú?¨Ð
¥èŠØ?Óދµš?¨Ð
¥èŠØ?so!ݵ§?xJæz•>ã?ïÙÓ!"i?xJæz•>ã?Å0PÊ;?Ä Ÿ»OT…?ê¾sëà
q?Ä Ÿ»OT…?¸˜Œ¶–±[?®úÐ[Ƨ?ììîi:èE?®úÐ[Ƨ?Ôáf7þ…=?±ò,J[¥?åLä½b?±ò,J[¥MIXED3FGL J1900.8+0337@BœæB¿˜1¿Û£Òm¾À7°]«¬Á•À9ñïÞIÍ?þ9ì$ÖÏ@›,ªØÜ%@͵^q$…¿ÓfÙJVê¿êt–Ë'–ô¿èèæç]п/âØõUNASNone@Ðª0U2aLogParabolanone	?A$Ca^w?JÑB¨ë«?ïû¶úÓpU?JÑB¨ë«? %:Oß?º5´Ø9g€?îÿݯ·×â?º5´Ø9g€?É#å ¶Ìä?°%5)陝?é·—ÒLÇ?°%5)陝?²ÀØ]Ùã?"bi0åÿ?í§ÿDæ†T?"bi0åÿ?fZì"ô4Œ?r×³î?ïé¥[¬?r×³î?ƒØX·ø7ˆ?¥xÌæM'?ﰞ(^2?¥xÌæM'?ˉÁÆp?¶þl'åA?é8<]Žd?¶þl'åA?…eÙT˜Ô:?q—ZC%@B?ïªhš"a_?q—ZC%@BPSR3FGL J1901.1+0728@DXÁTɅð?óþäǕUgÀ8.üóEºÀ:8*ù?ù霾è¼@
Óô²š@}…¬o	¿äen¿æ›Ž^RÕ¿çnÿ¿Ø¿évPŽã³UNASNone@•ºøFÜ]LogParabolanone
?ºãK©Ì—ž?À`g'è'û?죖ŠÆm?À`g'è'û?Éw6Qdg?È_¾RFÚì?é¢2k¦Ûæ?È_¾RFÚì?Ý»Éï³E?·0ÖVȧ?á"w¦]?·0ÖVȧ?à¶á† Ì?°‡}å{?ßԒ<ò¾h?°‡}å{?"6as^Ò?¬,›sÌF
?ïfLô#y?¬,›sÌF
?¦Ó½ìZ?¶5»óØø?îŸòÄX4?¶5»óØø?Ïá>ž'?¶»«à?è°\˜v?¶»«à?Á[®Á7Ý?§Ÿ"ô-Ù?ë©O²À?§Ÿ"ô-ÙMIXED3FGL J1906.6+0720@D˜±_ˆü"¿œ6‡P–ÆVÀ7îü¢}nÀ9áa£‰¤@'a–óÍ@
ØK)tª?ü¢üSøû¿ØŸtùÀå}¿âhÃQ46O¿ãî¯=B¿ê"G§"]UNASNone@ž'cˆe•LogParabolanone?Q&杨!ë?Vœ=®U?ï÷lŒßæŸ?Vœ=®U?ž?ÂwY3ë?º=RU@?ïìû?º=RU@?»¼ÚªŸÀ?ªotð×hé?ìˆ|ª¬?ªotð×hé?œoÈ¢·»?*b§	-?ø'?*b§	-?Sû
¸\uÊ?W	(0jgè?ïöy	´½?W	(0jgè?€çt¨Oh>?¢fžBìPÛ?ï¼b-5‡?¢fžBìPÛ?"^>ä<6.?'Ðv¥xÊí?ïeù›.?'Ðv¥xÊí?p>ˆÕ:ÕJ?]Å%ËUþ3?ï߂î±^?]Å%ËUþ3PSR3FGL J1915.2+0954@F9q!«K¿æ'"€zä£À824Òo£ýÀ:3î*ëf?úL0':+ @TYsŽÃ@Ú1'w¿ÕZ8äD…¿êÀ>/ÕI¿çÙŒ/n¿åó¡:!ä×UNASNone@·ŽAcLogParabolanone	?Ñi©(¥2!?ϚšJ™?çK+k­fð?ϚšJ™?űUWËC
?È/K¸÷>!?ꓪª
/>?È/K¸÷>!?áB'ƒìM
?·¦Ç])ÚM?Ý{°ø'eí?·¦Ç])ÚM?ß,¢™â-¡?±ª:@Õ?ài®³é0?±ª:@Õ?¤L­V±z?²ñ‡Ñ3þy?î»5*"8	?²ñ‡Ñ3þy?¡°ôˆÑÁ?²¢›d¹­?îäø›ö?²¢›d¹­?ÚcD`µªû?¼	/áf";?âÎ]Ï¥*ƒ?¼	/áf";?Á2¬4¿a?¬†"];ß?ë³TÿòÐ(?¬†"];ßMIXED3FGL J1919.9+1407@HZåÿ£¹®?Îó_ތè±À7Ȓ¡WÓüÀ9õ¦gÞ5«?ö{ëV¦@ܲ_Ž0@|®fÛ+_¿Ýº}ºjõl¿èR	c¥¨¿èqþÂé<¿æNkwQUNASNone@™ºÇË)LogParabolanone?ߟÜ}³£Ë?Ñn"ĺ?à0Á&.?Ñn"ĺ?æx¢ØÔåB?Í·asÀõ‡?ÓºNV5}?Í·asÀõ‡?܆™8íÿš?·Þ‰Z–«Q?á¼³c‰3?·Þ‰Z–«Q?é!;£^Y?¤(åUÉyö?Ë{r‡öž?¤(åUÉyö?ʉŽKT3«?Ç"‡!œ?é]œm*ó?Ç"‡!œ?ϐp‡ôÍê?Ë=ªiT‹?èãÞ̅?Ë=ªiT‹?ÜB,J8ï?½ø­ˆ0]?áÞéÿÚãˆ?½ø­ˆ0]?×õSa¯{?¶Ô‰¬'?äVO(B{?¶Ô‰¬'MIXED3FGL J1921.2+1506@HÝø>Ÿ?Ûi' hÀ86uT?ó5À:V‹"ÞQ?ÿ̒_"Žh@ƒjY5@´s0T¿Ä7·sÁ%¿ë§äO‡¿î•Uël¿îfžšŠZaUNASNone@'¬°O‹YLogParabolanone?MËøЯ…?cÍâ#[±Ð?ïøÛ¢S?cÍâ#[±Ð?£¯œP³?Á?¿žD'ðÌË?îÅ:½ÒD?¿žD'ðÌË?ÎHôïi?³XÜ?èmÂÄ=åœ?³XÜ?¬BÛºÙã¿?ö-¡×^T?î;ÒD—ô?ö-¡×^T?'™Œ®y¥ˆ?³²ÖÑ.?ïk3šŒ2Ô?³²ÖÑ.?…'èßúgj?¦&#	­Ci?ï«`\rWò?¦&#	­Ci?ͽòoÚ¿?·Ã'NÚI0?萃d	P?·Ã'NÚI0?w,–é|[?fÀÂBÿ/Ö?ïѦÒM{o?fÀÂBÿ/ÖPSR3FGL J1925.4+1727@J%]Äuq?äp?ÎL(ÍÀ8•+á/ZÀ:`Þ	53?ýj0'|G@Ûtä®jâ?ð¡ç¹b6׿Õ9n€ç-¿Õêߑt|¿ëÉ7»qõU¿ïÿâ–b­tUNASNone@"žÄ›¥ãTLogParabolanone?l]§ç?]Ç?Š»ûT…Ï?ïã¢XHÛ*?Š»ûT…Ï?¬rɐéX?À"*Š µö?î8Þc«©š?À"*Š µö?°ºvj|I?¢àRA"•'?íè±=`nç?¢àRA"•'?ÀRwÏ¢ó"?£Œžf5}¶?ëëbC?£Œžf5}¶?h"`}û϶?¢ž·0²?ïçkŸ"â(?¢ž·0²?ŠãÖ¾µ?¦¬RÞ
*Ð?ï"s´¥*?¦¬RÞ
*Ð?'Q]DŽ¯?'¾]ºßÿ?ïmu¶?'¾]ºßÿ?ŒD³,Jˆ?~¢=ŒÇ?ïòí%f?~¢=ŒÇPSR3FGL J1928.9+1739@Jm[[Õ?}&3ò"'À8imOŽ³À:4››ÒXþ?ú@ÈÍcˁ@òlÃ!Ó9?úgRژgj¿á1ç)€"¿åQƒ8aÎÛ¿åÇ[sÄ¿íµ²ÔÔUNASNone@›¶úÇË)LogParabolanone?–sɈj?Ÿ¨æ.@ÜÉ?ïLg¡œ>Ý?Ÿ¨æ.@ÜÉ?À}N'è®?Ä4&Uݵ±?ëûà¬[EÔ?Ä4&Uݵ±?Óí½‡?´["zÞ³ù?æ	ut¡=?´["zÞ³ù?Ö9óÑÉ`Ý?®ÕÄ«ËÉ?äãO'?®ÕÄ«ËÉ?SãÝ¢—uü?ZuÜqv¸?ïöe®?ZuÜqv¸?˜"ù‡ðî£?ª'W@€9&?ï;`3¤û«?ª'W@€9&?¹r­­³é?¬µ»"Û?ìѪJI'Þ?¬µ»"Û?±ÛzcÕZ?™ññÆí"â?íďÐÜÀ¥?™ññÆí"âPSR3FGL J1946.4-5403@u~6z—À=ûH
[À94ìð{(À;µû-2h2?þρËDz@
r©rՊŒ?ø·÷'¿7?×¼ê×yÏ¿à܍¸'¿è½ãJ' V¿ìýco³c'UNASNone@ŠaG®{LogParabolanone?<Oïw[-?OƔ4/HÄ?ïüvÜEˆ?OƔ4/HÄ?µw*ÀL?Å;r‡öž?í\q§ÿ—?Å;r‡öž?´­‡¿gäŠ?¤
ƒm†‹ã?íjOéÈ?¤
ƒm†‹ã?¤Oç…›?‡íãB¼?®Nv?‡íãB¼?Wô±	þ?ZœÎÂBGµ?ïôvrß+Û?ZœÎÂBGµ?£³)¢=?¸«Ï™^J?îÇÆä*Œ?¸«Ï™^J?£ûØ?›¤³u…4ª?îΎuú?›¤³u…4ª?i©FyM×?]LÆ*'ç?ïæV¹J9	?]LÆ*'çPSR3FGL J1949.3+2433@NšiƒQY¿çCM\ª%À8ÍSù|X@À:¬°',ãŽ?ùƾ•|@
ï/"Ã?øâÞ0¿Åçö-z¿çnKŒ	Qý¿èJ6F°_ü¿ïýÌø$ÙUNASNone@•z!@N¥LogParabolanone
?¦v"ÕìMt?¯´+BÞRÚ?ÂØ4è?¯´+BÞRÚ?²9ÞhU©Ö?¿Tï+؇&?í¸Ä3:õ?¿Tï+؇&?ׂè=Ò¯¡?²òSÔcF?ä>‹á¨0?²òSÔcF?ÉHTBï¶?¥GPœ?é­ÛêïD?¥GPœ?ˆ,NÜiÊ_?¨-"b%¤?ïŸNĀšg?¨-"b%¤?)X¯g¸Ö?§°Áx-O?ï~µ:'€©?§°Áx-O?˼'šfö?µ
0÷ÂåZ?éÛYyæB?µ
0÷ÂåZ?—@Eò%íh?Õ—Ò2ª?ïEýÐ¥ÊT?Õ—Ò2ªPSR3FGL J2017.9+3627@R¢ª:э&?ÚIECVÀ7tUóQ›ÔÀ:1GNs*š@A(¯ ¿h@
{œüOœJ?ö"|ôÈ>s?áô3ˆî{ž¿ßå: &)ú¿è§°[…•^¿ïh]QóEeUNASNone@™ÚXüPHLogParabolanone?T«'?œTà.4æ?ïÿUZÐ["?œTà.4æ?¢`Ny~ª?½«.Y7\?îÞ)úánV?½«.Y7\?}G;ÑX÷å?‡Wbáx_Ë?ïÅqˆGP?‡Wbáx_Ë?l-$/??TÐâÖÛ`½?ïãÒÛ¸*²?TÐâÖÛ`½?'û¡%_gŠ? *M¢¯h?ïþ€F}? *M¢¯h?‡9¹Ù+à?¨7Ànl/®?ï£ċÏ?¨7Ànl/®?rTkÈÁ‰?bçVòpA|?ïÛW(¨79?bçVòpA|?<^0û‰}?0X ¤'ðÆ?ïüt:™¡?0X ¤'ðÆPSR3FGL J2023.5+4126@SÐ:>À/0@»|,ÑðÀ8"Ð=1À:pñÒ?ÓU@hòbˆ‹@ ŠÒ+†l@BMec‡¿Ü:&ôØÑà¿æW?ÁQ!¿î^måû`οأ>ÍUNASNone@"#O¿ÆT
LogParabolanone
?Öc3?ŒKÂ?ԇå	¸=?äÎf`9Ú?ԇå	¸=?²n"?Áõ[¦Ö?í¿_ò.?Áõ[¦Ö?à8õ|:Ûk?ºj&"¬^‡?ߎŠI+?ºj&"¬^‡?ÅhEÌñhk?®K"_aµ?ê¥îŒÃ¥å?®K"_aµ?àʏþÎ?Õc{dû,\?ßÀjàòd?Õc{dû,\?'f\³è­Ü?¬6€³'{?ïlÍa?¬6€³'{?àw˸b?¼Õm§š±?ßhŽÅç<?¼Õm§š±?œå̦uðÔ?¢R•—4<?ïњçÍY?¢R•—4<MIXED3FGL J2024.6+3747@Säy'¼?°«'¡Æ3À8¢×áÓÅÀ:vXò	8?ú*W‡PkÓ@MjàɃí?ý©£A«q?ƒÆó¿ë ǾΏù¿á8ÌÈ5‹¿êú¿»ä"ŒUNASNone@‹YŽuyLogParabolanone?Ô»¤ƒ$¸?̽ÞAB"?å¢-¾mþ$?̽ÞAB"?Èð"¹FCl?ǜlÿÿ÷i?éÃÚÑ®o%?ǜlÿÿ÷i?àU¡¹'w*?´ÊÑ"Ìþ?ßT¼ŒÛ«?´ÊÑ"Ìþ?ÝO‰%À?®=æ  ƒu?áX;yíp ?®=æ  ƒu?°´À…XÔ?¸™õ½ýi1?íé|¸[&?¸™õ½ýi1?©M¸ùéâô?´xð¬7òY?îk$po A?´xð¬7òY?Òì½Ïêö?·Úڋ?æ‰û¡
…?·Úڋ?ÂÉÜÍ Ý0?¦žû¼Ñ‰?ëMˆÌ—È´?¦žû¼Ñ‰MIXED3FGL J2026.8+4003@SŸ}€^_1?ðf¬ƒ§ÀÀ85>˜ÂEÀ:S½ei?ýöâõÙ@ð}0Ò?þ̌ÐÞT_?î´®>R‡H¿ê³¯J¤Ð¿èÏÀG¶Öt¿æQA~6UNASNone@†¥ýŠÚºLogParabolanone?ċtcYe?Éçke	™?êÝ"çé§?Éçke	™?¾Õ]CkÔS?Ïz.ÍÑb?ì%TW'…v?Ïz.ÍÑb?àÓ'Úºv?¹ÞÝÛèɃ?ßÊY°J‹?¹ÞÝÛèɃ?ÔïkÎZX?±{«òt—¦?åˆJýÒÔ?±{«òt—¦?»R*DL58?ìßWÐ?앺·vyY?ìßWÐ?¢†nÓúó?°ÊZùÌÝ?îי¤â?°ÊZùÌÝ?Þê}ÍF€?½ôüIo¾2?àŠ·Á\À?½ôüIo¾2?¶YKzƒ¨?¦œ
×U¨?í4֐½Io?¦œ
×U¨MIXED3FGL J2026.8+2813@Q5éÍ³}ÀK5°»õÀ9˜d
ƒ À;:†œfÓt?õà—Ê·sÊ@ᓿºëy?ùj§ŽN⼿â2kü¿Òs=idj¿ï†)ñk¿ïýGwtUNASNone@Š}ÔA5TvLogParabolanone?·[ea›µÚ?¾D°H²¡R?í"S•…?¾D°H²¡R?»\´Bߚý?žWá¾?ì"iw¤ ?žWá¾?܂ÿ€ËŽ×?´Ó9ôj?ᾀ?š8•?´Ó9ôj?Íõù- C¤?«Q`3¶)·?肁´—ï?«Q`3¶)·?–…&2(M$?­ú=|bQ?ïKÖÎ`ÿ'?­ú=|bQ?"/«ý?©ÖÜ
Ñkø?ï_÷>^‡?©ÖÜ
Ñkø?é¤Óç¸?«êç².Ðs?ë–üË?«êç².Ðs?™38ÅÜ?€ê‡=Ž?ï{6gE3'?€ê‡=ŽPSR3FGL J2032.5+4032@SàÞ~¥øM?Ü
#$G]À7 dJ,süÀ:*†ƒ<`@÷øµ"@;U«3@˜­×êN¿Û‰å—=¿èÒ~?ԉã¿ïÿÌÔY‰?ïÜn~Éð¶UNASNone@Še­à
qLogParabolanone?íhñ"äÔ?Æ&àÎ{<{?´¿ØvèÙb?Æ&àÎ{<{?í3iÕÓÿ?Ë,/Y›
?¶g4²-G?Ë,/Y›
?âUÃÎÌVZ?·~'zm,Ê?ÛTxbgSK?·~'zm,Ê?﬊Â2·Z?‰Šæúý5?"ÝO} ý'?‰Šæúý5?î~®Œÿ0?»e.Ág?¨@Û?»e.Ág?ç
HmWp?Ô´Lóx³?Ñåo%QÉ ?Ô´Lóx³?çOÆ3MÜ?¶ë;r¨Ü0?Ñ`s™eþH?¶ë;r¨Ü0?íÖ¢;S¾?¿ÐáÍm-?±Jî'Ý<?¿ÐáÍm-AGN3FGL J2032.5+3921@S¤´·,Q˜¿Ñ0l娶À8,Áúá³À:T
ހS?þ/}Ç/%@3'W°ëñ?ûÛ@bƞµ?ՇW€M÷¿ä¥fÁÕøÅ¿ê`*èêmO¿çºº•VƒUNASNone@™¤—ö+kLogParabolanone?°£ÆÉF"?¸Æx[7¡?íý+‡BT
?¸Æx[7¡?±õZËj±?¿ö§oMÉ??íÁT¦ h@?¿ö§oMÉ??Ø-ó¥¡?¹i%}F
?ãûé-/}?¹i%}F
?ÈÖ¨
ÿ'?¥ÓD$ï?éÊUý@:¶?¥ÓD$ï? K%ÐñŠ÷?®TO™ˆ©?îûM¢¹í'?®TO™ˆ©?"Oöº6X?©E­D'w?ïe€O.M?©E­D'w?ÖëÔ´øš±?½h\N¤B?䊥ƒ²¨?½h\N¤B? ¤}ñoô?†	Ÿq?îõ¸ öÎ1?†	ŸqPSR3FGL J2034.4+3833c@SŠOv_Ù¿ð®â5ꝘÀ8^ìÔªÀ:‰Ë—B§D?ú&ñ–…½ð@›àÆ©È@;¢F¨0¿×¯‰Uw¿ë
¬ÑÚ¨®¿ë †?A*忁
cgÞ>UNASNone@€•9ÀëíúLogParabolanone4?áAÒ]Zy?ҁ†s;?ÝÇ|[EK?ҁ†s;?聠*.
?Ñeƒ
²Ã?Íù}‹WGÌ?Ñeƒ
²Ã?çBatD¼?³@ƈ~Øè?Ñ{=ãv‡?³@ƈ~Øè?ìK¢+t´?«[x;nù¯?½¢î¤Z_>?«[x;nù¯?Ë5÷³ˆ?Çu¢¶ ?é2'Sù?Çu¢¶ ?Ô'~.Y.Å?ÒÊ%c‹/?åì@èÓh?ÒÊ%c‹/?âQ/²ö?¸¢Gœ<t?Û] šçé?¸¢Gœ<t?á1Lñ @Ó?Ìlèðˆ­}?ݝf¿~[?Ìlèðˆ­}MIXED3FGL J2034.6+4302@Tq?l&š?ù¨·^¦~"À88;·f3À:bþ;â?ÿaºÅc@
ÉY;°…C?ÿ¾–EÒB¿ãRêCçG¿ã¤Š÷t¿ëpK&L£¿èáX'€_PUNASNone@‰"ÃÞ灄LogParabolanone?–Š¨q?¡Ã9³ÒkL?ïKª¼'Ô?¡Ã9³ÒkL?§åô9m÷å?¾rém¹¹?¼M£¢?¾rém¹¹?Ú#NFDC?µ"…MkÊ}?âîXõÜÝÞ?µ"…MkÊ}?´±0µÛ?–:YÈ<R?íiÏÞ5f%?–:YÈ<R?‹(½M"ԉ?"âÁ3o Ó?ï"]
Ù3?"âÁ3o Ó?6OÃß?¨¾u˜žÌþ?ï‹÷&‰ùá?¨¾u˜žÌþ?ҒN~Ìö?µïÞkºöý?æ¶ØñÀ™…?µïÞkºöý?/M)T¡?q°îҝÛ?ï»BˉÞ?q°îҝÛPSR3FGL J2035.0+3634@S(ˆ&ªŽ´À†»øiÀ9°à<4À;
-åìY?ü«äåS@²ìì§Þ?ÑNÓã:?ïêÖò"[3?™é¢à.Y¿Ö¡CU®÷é¿ï0#ëËUNASNone@ ¡ŽÙ‡+LogParabolanone?£^¦ÓŽ¾ç?½'l4X?îÊ'¹U¢?½'l4X?À3Tô¬˜X?Ąg/†wË?ëó*ÂÔÙê?Ąg/†wË?ÁDd—óëä?«ÖÝ_Ö¥?ë®æÚ?«ÖÝ_Ö¥?ÑjÜlÒç?²Óºu÷±?çJ'É–Œt?²Óºu÷±?`i1|æº?²UL:½¬y?ïº~[z¥
?²UL:½¬y?°8.§í¡,?½#²TÙÿ™?íøú+
J?½#²TÙÿ™?À¹?á0Jå?­Ö"ZA?ëÑ°³íG?­Ö"ZA?·ÜA﭅0?§°ÒÙÞ°?íwÁá
?§°ÒÙÞ°PSR3FGL J2038.4+4212@TaÄØì–?á]iR‹¾À7ö;¤ñ¼pÀ:ûwÛð?ÿSÊ7F=Q@'<§P;'?ýC7àlõ¿¶ÕA™(¿åæà/'N¿ç°—já¿é8‹ÛÀÛUNASNone@™Ì™‡+LogParabolanone?l3ûÕ*î±?{üB7ˆY?ïãÌèܒ?{üB7ˆY?«,KN½:N?¾¨(VúýQ?îM;Jêñ?¾¨(VúýQ?ÐN??³µ`WU<Î?çˆ23Xòà?³µ`WU<Î?ÀZ?•Ûã°?ÔÊF?ëép‰?ÔÊF?`gÖ5#ËÔ?cö$?ïï˜)éÄ?cö$?(ŸÐM1w?¨œâZoæ?ï~»¦ÑÄ?¨œâZoæ?¿8ïÏu
?µÎÁix[à?ì˜â^?µÎÁix[à?•Ä»Î{7T?Hgœú%»?ïQÚ!bêö?Hgœú%»PSR3FGL J2039.4+4111@T5¨mqó¿Ê'¼£nÀ8û'²õ‹À:AàLÜQ¥?þìñÓA†@…̘Ih@ê:Ì.Â5¿×´È\ƒAF¿èPÎáÇR1¿ë58~v¨~¿äÝaeÎUNASNone@‹Ô®]á\§LogParabolanone? zºrŒwc?°ðñ¼'ºO?îøTX­ý:?°ðñ¼'ºO?¯Š°«?¿v»ÚGoç?î^u"/?¿v»ÚGoç?Ù£v'àªá?ºÙòËË+H?ã.D쪏?ºÙòËË+H?Ä÷øŒ:­È?¥…ÿ&œ|?êÂÜñTŽ?¥…ÿ&œ|?—øú»
*ã?ªÝ"o®É?ï@8)ðœé?ªÝ"o®É?"½m²€³?©ºnU'?ï{Z"­Š?©ºnU'?ÔÀ×#p{?ÁÁ"Å!1Ô?埔nGÂs?ÁÁ"Å!1Ô?˜°š? )©Lk?ï?ß"²(ÿ? )©LkPSR3FGL J2039.6-5618@uS²þÅm]ÀB"Ùý6÷äÀ8ʇkŸ‹À;O3·½q?úfý4Ñ@Y…kE-?û-x¦¯×Ÿ¿ÑӂMø†d¿ÝÝ'ãɾz¿ãˆã˜/% ¿í×)5óUNASNone@Ž²WÛô‡ýLogParabolanone?ymõSBÜ?Œ	Õ£?ïÍ$ç{'?Œ	Õ£?¿("ûÊ2¶?ÊðÏ´;d
?ìï`†¹©?ÊðÏ´;d
?ÉÁº•<½¡?°ÔR±‹z]?鏑Z°Ð˜?°ÔR±‹z]?´@		²éô?"¶ÎÍqÒ?íwþÞå¡?"¶ÎÍqÒ?c€!?k¯~ýÈØu?ïìýç!?k¯~ýÈØu?¬È¢ÐåŽ?¾Ã
ôŠV?î3uÓ
P?¾Ã
ôŠV?³$ïžj?–"pŽ(9j?ïfØYÑ`?–"pŽ(9j?}T'P"@•?mœ"¸ô?ïÅW±}ø?mœ"¸ôPSR3FGL J2041.1+4736@U…Ó™o¨/@±€%TM_À8+Yª–AÀ:ÇvË8x?ûöžšŠZa@…4"@ÔŸgd¿×bYäfü¿äÒø/§Ÿ¿éN9¥Ni׿ê(±Žû'vUNASNone@"PÊôðØELogParabolanone?҅–¶ÿõ³?ɦp
K€?æ½4¤€'?ɦp
K€?³½@‹ã?À;_Z65?íˆW€?À;_Z65?ánüöÇXU?·M
ôN4Û?Ý"qOV?·M
ôN4Û?Êk–ÏÃTÝ?¢ÐÖY®ì?éeL*É?¢ÐÖY®ì?'ÿ*R?"*SCQ–ÿ?ïoü/êm?"*SCQ–ÿ?—‰FøþR-?®/‰¬!í¢?ïCµÈ¯?®/‰¬!í¢?·>jÃ\$ˆ?­Öçyh¥?í2§Ù3Ÿ?­Öçyh¥?œZ0ß,1?ƒí´%Çqç?ï.yžw?ƒí´%ÇqçMIXED3FGL J2042.4+4209@T{ªOÊB¯¿²;X6LîÀ86‹ò)ôÀ:UÊ! áø?ú)Œì7 S@GØ4ß۝?þíâ¦Ó¾Ù¿Û¦IŽ‹Á¿èq®0Ý÷¿ã¡ÄZ"Ó0¿éãP÷,rUNASNone@˜"ä%®æLogParabolanone?ÎPâÿýQ?ÐâãFЎ?èkÇ|¬?ÐâãFЎ?ÃÄَQ<?Äñgû?ë<ɜk±?Äñgû?áåéšÛ}?·Ô˜Ñg?Ü4-ÖÊI?·Ô˜Ñg?Øo&9¶Á.?©¾Ö\F«?ãÈlã$Ÿi?©¾Ö\F«?¦óBý1—È?³·|m#?îËÐV!Ó?³·|m#? w³Bq›w?®G'諏5?îø"Ì!˜?®G'諏5?Ñv€o§â?¸Hr?çD¿È,?¸Hr?¶`¡¿þ"?™Kúhje?í<s묃N?™KúhjeMIXED3FGL J2043.1+4350@TÕßeUÅ?ëﵩ-‹À8"Íui8©À:· ×æÜC?ùƔ·1¯û@wOz;°Z@ªWk÷ ¿Ü7âȕ8?¿í§"€"¿Ø–§XÁYž¿î"i$ösSUNASNone@}St!-wLogParabolanone?Ö´q«WËÞ?ÌGFê¹á|?ä¥Ç*T?ÌGFê¹á|?»}ïÞ¹x?ÂúŸŽ%G7?ìPB(Ñ?ÂúŸŽ%G7?âü:"Œ¥¦?´ÙJ®ç'?ÚŠÖæ´³?´ÙJ®ç'?Öã"ñä*Ú?±ÛJAïC?äŽ=‡
ê"?±ÛJAïC?¿¸³©ÿÝ	?Ã&se0Ë?ìéŠÀ_?Ã&se0Ë?¢…•Ëk¿:?³×²4Y®?îצ£ ½?³×²4Y®?ØlXw,J?¹Ý¦A{S?ãÉÓÄ@iÛ?¹Ý¦A{S?¿çDÙ_›?°ƒÊi¢ù?ìdÔ­?°ƒÊi¢ùMIXED3FGL J2048.8+4436@U%+ÓÃa?át0‰4LjÀ8|@lÚÀ:à&¶ÁÉ@!­ÎYê­@"R£eö)?üîԞþ2u?Ç`MŸ½l¿çôò"䣿첻尿ïÿ" ¿mUNASNone@…xF?LogParabolanone?¼Å~¾¸¹?À/ý–ú?ìgP(-èé?À/ý–ú?¥Òæá-Ôe?¾[UCÜ×:?î¢Ñ'¶(ú?¾[UCÜ×:?Õ%6'°"?´/<:A#?åpíd¶§¶?´/<:A#?­;é)?Ž–X̓Ϩ?î,Amnԅ?Ž–X̓Ϩ?¹7&h?ÀDސ]t"?ìޙ""ó?ÀDސ]t"?Œ•æ-\_?¨oì×A5y?¨YŒ?¨oì×A5y?ÔrÉÈØÃÈ?¹
™kʟ?åƛ"ž?¹
™kʟ?}NN¨Î,?j?öRëª?ïÅcbŒ"t?j?öRëªPSR3FGL J2103.7-1113@BíÐ|"µÝÀA6)Çy¦µÀ9Í#¯1±À;¿VŸI?÷9`üÅ
@N¸Ê·H×?ñЉB37?ïÿxùsŸ¿×¨ùD5J¿â7îÕú⤿ì
Bùú­UNASNone@—‡•L˜_LogParabolanone?Άaó(ñ?ÊWY}Ç?èx^gƒ5Ä?ÊWY}Ç?ÛS8?ÎZ*Á¨4?âyÖ8cý?ÎZ*Á¨4?Ùö%í:?¹E¼¹^z?ãíxq‰c?¹E¼¹^z?à×ôf2B?°u­¶o?ÞPß3›}?°u­¶o?´Æ[¢ö·?¹ÍKҀ?íg4‹¼¥ý?¹ÍKҀ?Ȍ	ìgó?ÊÏ°Ï7®?éÜù}"æ?ÊÏ°Ï7®?½kñßo«?°KÏï{Q?ìRŽAÄ?°KÏï{Q?Äç²Ãـ‡?¨Ã5Óù?êÆO	ŸÞ?¨Ã5ÓùMIXED3FGL J2112.5-3044@-Ì`RP/ÀE9nÀY!À8¯¨tþ¯žÀ;N%@+i:@ABŽ@•ä¯—‡Ç?ñĐ£PҀ¿ºTqu§æ¨¿ÐSF"ã!M¿áG¡>Ô|¿ïÿù_|è3UNASNone@'¶¡ÊÀƒLogParabolanone? áz-Ð?±¼õ1æo?îÿ¡ïºž³?±¼õ1æo?DZiÇl¬?Ò}¿ZÒ?ꥎ;äÕ?Ò}¿ZÒ?³2Ïùç2?¤2XÐx>Z?홦¥F:?¤2XÐx>Z?¯‰AÞ·e?"²èq?îkïÙ:?"²èq?¯§àªj?ÁÞâT"¢Î?îU',Yi?ÁÞâT"¢Î?»…Ul'?ÎÉÄã'
?ìU^'m½?ÎÉÄã'
?¥E9ú?¡
"B×·?î¦/û¬op?¡
"B×·?†.2èGŸ?u¥ùªÍ‡Ö?ï§G7¦²?u¥ùªÍ‡ÖPSR3FGL J2114.0+5239@WWn.±Ä3@ßT•Ð·À9,Òn¥ÐÀ;ÚPp[?öaÅõæ@)0¬›)?ô"rþ¥7?ïþ,0Á®¿çX/ŽZn¿ê\¼:û¡¿Ù­k+$ÏvUNASNone@‹D2ÊW¨LogParabolanone?î|Ì{¼?´ÊõçÎ/ù?®îè1€vJ?´ÊõçÎ/ù?ëßÎKŸ]?È6-Žƒï?À€Æт‹'?È6-Žƒï?êr^»2Ä?®—wÿ‹¨û?Æ6…5øñ?®—wÿ‹¨û?ëÔúùäe£?¦l §ªÔU?À¬nis?¦l §ªÔU?ë3Ë>àÄ?ÿR¬±_š?Ã0Ó|ïó?ÿR¬±_š?àv͟¹ ü?Ò31;ó?ßdÀ¾?Ò31;ó?é:@µ?±MÛÉ®¤?ËýÁûý+?±MÛÉ®¤?Þõ
†Ê<­?Ƨáy	ß°?à…z¼šá©?Ƨáy	ß°MIXED3FGL J2117.6+3725@T³ {5+À Œ$=Ìê)À9´ã¡ûhÀ;[«Åìû?÷º¢˜›Â¿@ImÖr=	?ÿÚ.ÌHî¿Å~Þ]ÕŽ¿å))'¿éˆWHÕö†¿ïÿÃ	ÌUNASNone@'²ÓŽóMjLogParabolanone?ä$5	TÆ	?Îjˆkì.´?×·•íVsï?Îjˆkì.´?º›&ïO{
?Âùâÿ÷?쬛"Ÿ?Âùâÿ÷?áQUތpo?µ&pPKÒ#?Ý]TBç"?µ&pPKÒ#?Ðb4·†ƒV?¡»Ë†q`Ð?çÎå¤<¾U?¡»Ë†q`Ð?½2ýî­È%?À¢¶lÁ—?ìY B*Fû?À¢¶lÁ—?š¨±~r	?¯+Yo
þ?ï*¿:Êà?¯+Yo
þ?Ç¥~4
x¹?µÎ_¬]Û?ê rü¡Ò?µÎ_¬]Û?žÅz$?}Øʌvµ…?ï߉Æpp?}Øʌvµ…MIXED3FGL J2125.8+5832@X¯iì,äe@Éú©u°À9'][û©YÀ;ˆ*…È?ö9B×@I@MãÂË ?øÉZí6yº?ÒÀÖc=Uæ¿çmõ*ÜD¿ë:¿»Óg¿ê¨»VO9UNASNone@ˆ0÷€4mÆLogParabolanone	?éכ7Üî·?ÂäJ9V…??È¡" ŒE&?ÂäJ9V…??ã£æ‹SŸ~?Íe
×ۄÝ?ظ2éXÁ?Íe
×ۄÝ?çxP"ý<?²ÇÂZǤ?Ñ_ö؇?²ÇÂZǤ?äµô`1?«Êr[ew?֔?àâ?«Êr[ew?ß+ƒD Hþ?Ύª¿ºH?àj>]ïہ?Ύª¿ºH?ÆãÀ"G^Ó?Ƌþ;â
?êGÛ.(K?Ƌþ;â
?ÜÖÓ	©ï?·iÕL´IÚ?ᔞ6{+?·iÕL´IÚ?ÿ ÷(bl?¬Úlœ±2/?ëÂ5çe?¬Úlœ±2/MIXED3FGL J2133.0-6433@t‹Ò½<6ÀD¢VÿÁßÀ:@ËLš†À<	—@G?ùþð`z¿@B°'¿7Ž?à~ð~‹Sä¿á'òWBT¿Ã4Ì}‹¿é@¢¶½…¡¿ìiµþK—PUNASNone@™‰½¿HÌLogParabolanone?Ty©åE?¢§zŠŽ""?Xk§?¢§zŠŽ""?à©Ø9ó†?ÑÁYVˆwÞ?Þ¬OáŒõ?ÑÁYVˆwÞ?ÔM! '—
?·V&{øp€?åÙo/ì4z?·V&{øp€?Ù×!t™ÚÝ?¹KôúW8e?ãoE³'?¹KôúW8e?›;ÿ7G? 9LXÇb?ï&'ÐEÈ? 9LXÇb? f²'1?ȾY'¹g?ëWæS[œ´?ȾY'¹g?Ëõa&Ǧ.?²4ÚôŸýö?駶Nu?²4ÚôŸýö?©½
;\f?¢ƒzå¯?îd/\†Ê?¢ƒzå¯MIXED3FGL J2206.5+6451@Z¡ï^Èt@'W«¸€À92FÀ:ü¹kÆøw?üÁ"\Ð@ef»ü@…újꯌ¿Ïøå!µåÞ¿çғâº8º¿êŒœ",r¿ïÿ"Ó¿¸ÆUNASNone@‰ìô!-LogParabolanone?¼}PF®?À{l2\?ìoÐUÿw*?À{l2\?«Š‡Ç£ÜØ?À¶‰ÛFÉN?îGWƒ…Â2?À¶‰ÛFÉN?Ûß¾jù
?²Ì饁"?â ʃyû?²Ì饁"?«û×>z@?‹³ï둲:?î@B‹üß?‹³ï둲:?¥ËéÞ?²Oõ9?î£O'sìr?²Oõ9?"ta˜ú¡í?«zàt ?ïd\óï¡?«zàt ?Õ¿lnŠ™™?µ–nð7Zì?å IȺ³4?µ–nð7Zì?rq³Á‹˜?^
‹¡cÞf?ïÛômáÁ?^
‹¡cÞfPSR3FGL J2212.5+0703@Q/‹«`kÀCHP½‡µlÀ9nv½ÌÀ;™FéÉ\Ö?öÙù΍—-@4~…l?ûHÙÉà^¿Ö$;"Ì"¿á*øú¹U¿ä7û"i¿ïÿåFúUNASNone@Œk…¸RLogParabolanone?âÂ+)Š¤?ÍS/Á¨p;?Ú{©¬ê·Í?ÍS/Á¨p;?ÙBæ'ff´?ÍAR:Šj}?ã^Œ·L̦?ÍAR:Šj}?à×~N?¶ၘNž?ßÆQcó×?¶ၘNž?ß.ˆ}+i?«
-†"0?àh÷»ÁjL?«
-†"0?ÀDªÌ>Sð?Á¹bj`út?ëîÕLðk?Á¹bj`út?¾ríÄzT?Á·
Ÿ&‡?ì1¢Gpµ}?Á·
Ÿ&‡?¹>ä<6.i?¬6%{ƒ$?ìØ#x]½S?¬6%{ƒ$?¼ŸèƱ}?ž¥PGpJù?ìlç)ß?ž¥PGpJùMIXED3FGL J2221.6+6507@[¿Ž`€@ÂQã!¢èÀ9gJöžWnÀ;ç½?ùû÷²©‹@M;G(Þ@…xì?Âyð‹1»©¿æb©\h¿ïÝÂ凮¿ïGKI½ÂUNASNone@…5IîËûLogParabolanone?Ò¿æ¼Ú]Ñ?ͨ'…Ôë?æ ¡'Ñ?ͨ'…Ôë?ÆQ:¸Á/¾?ŃqÓÆ«?êk±QÏ´?ŃqÓÆ«?á8#íðÞÐ?µ5T[!q?ݏ¸$B`?µ5T[!q?ÖA9EÆÞ¡?¬†Ñ;­'Y?äßc]¯?¬†Ñ;­'Y?̯
`Þ¬?ÌәÝ-ºp?èÔ<§È}Õ?ÌәÝ-ºp?§j1®*?´‰çHCÔ?î‰\åU§?´‰çHCÔ?Ù	¨93l-?¸J
Ó'5Í?ã{+ãfIê?¸J
Ó'5Í?§ø%Ùííe?"÷ãýh?î€}¢Sbº?"÷ãýhMIXED3FGL J2221.7+6318@ZÁeUÅ.s@›¡±–À9(‡%ùŽÍÀ;&'d@ò?þQH,>¢R@
;ÏWì{?ü2ßã«¿Õ4o)>ÎÙ¿ç¡äÞ³Ìm¿êüÇ`sª"¿ç"îrA™†UNASNone@‡'£S&LogParabolanone?¾Ïƒ>Ï?µËîg?ì&˜=<æ?µËîg?¯o!;ˆ?ÀBF'qÃM?î	
ìbû^?ÀBF'qÃM?âdp«Aja?¹Þòzl"ã?Û7©}+>?¹Þòzl"ã?¾Ï¼¢¡ð? g(–í¯Ö?ì&k«Â? g(–í¯Ö?ÅH€JiÊ?Æ`¢âÄ$?ê­ßûíe?Æ`¢âÄ$?'˜Ü=F¡?ª®\ڂŠ7?ïk9Ë?ª®\ڂŠ7?áqå%M,?¼áÃÔֆŠ?Ý5µïe©?¼áÃÔֆŠ?ˆõք§1?|–OÍå?(|²?|–OÍåMIXED3FGL J2233.1+6542@[UîËûµ@>Û<ÒfÀ8ɸKgÝÀ;ØWDŠt?ú³
-ºù;@¯}W´@uàŽ ¿á"ŸÇ±¿æ±.–kfֿ놥¥Z[Û¿îljˊfUNASNone@÷uY³Ð}LogParabolanone?ÉÉúנּ?ÃT«d.?鍁xÄ ?ÃT«d.?´¢"V"ËÏ?ÁEùDc?ík¯ué¦?ÁEùDc?ä+qÈÅ+?³÷~#·ä4?ÖÅ©nu©?³÷~#·ä4?Ɲå	üÐ?ž|al¯ë;?êX ½€Ì?ž|al¯ë;?¦;¥¦íd?©€‹˜´s8?îœE¥ž*?©€‹˜´s8?™ê#`1Œù?®ñ95Ç?ï0®äâö¸?®ñ95Ç?×ÅÓCg?¸R@ÞÊ?äs^Lx?¸R@ÞÊ?'	úvž?v{åeŠGf?ïo°/ÄO?v{åeŠGfMIXED3FGL J2237.9+6320@[&E^®â@öj}L[ùÀ9Z¼ËÍÉLÀ;S:ঞ?÷¼©ÑË\@ T´àó@ü«¶Q¶+¿Ë1Š$Z¿¿ìˆÐí*¿äÉiý
¿ì¦
ÆŪLUNASNone@j"Á*ØLogParabolanone?ÒùS^Ýí?ÇŸÃw?æƒVP'	u?ÇŸÃw?ÀhÒÔp&¦?¨‹bQâS?ëåËJãöW?¨‹bQâS?ã{DzÕÅ?²ð°+×IS?Ù	wÁ
Tu?²ð°+×IS?֌6•ÏpÒ?¨<¼Èh?ä¹äµG—?¨<¼Èh?·Yºm"
?¶B+é½ÉO?íȲi|Ï?¶B+é½ÉO? }¸‡Xió?°Þßw^G?îø$wa>?°Þßw^G?Ü!p­è7?·±ØÜ|M?áïG©ýd?·±ØÜ|M?®‹~(?'à,*Ibq?î·H+<ð?'à,*IbqMIXED3FGL J2310.1-0557@Qlvò¥¤jÀLø(¡ß¹9À:b8š{@éÀ<5[½•ø?úØ1rìí@Pž¯®?«ɔ•)?ï¢Z´ñ'º¿©‰ì	!¿åèg™±`¿ïÿyOw6˜UNASNone@—I^쿱[LogParabolanone?ÏN=šë(X?ÔÕi•=ú?è,p™E5ê?ÔÕi•=ú?ßý×[Æû?Ò¤[…s<?àqR'?Ò¤[…s<?ʶöäè?¶ ïïGÛ?éRzFù†?¶ ïïGÛ?ØÈ>	rfò?¹²|МKa?ã›àûḞ?¹²|МKa?Å՘iT¸?ÓIŠ!p³?ꊙåªûR?ÓIŠ!p³?Ï*#'ÿG?ÐÞa<Ï·?è5w6 .?ÐÞa<Ï·?¾L'ØHð¤?´D¥éîx?ì6mÄöáì?´D¥éîx?¶ç(L "½?¬¯`Š—8º?í#ö•6ø?¬¯`Š—8ºPSR3FGL J2353.3+6639@]M©?)
»@½?é$À9)ölÙG/À;O{ƒ.J?þCaƒ‡4@
J^Èã3?þi™aܔ?ÒéQ؄*¿èñôgN }¿ì€zŸê|Ç¿í›>ŠTWUNASNone@"¢S÷ÎÙLogParabolanone	?tÔ.Lbéã?€ùnõ5á‹?ïÖW£]›D?€ùnõ5á‹?¨&ˆ¸VB?ÀðkÁm?î}—t?0Ü?ÀðkÁm?ÔÈãM?³âL¯ð?åÀŽ{Ù??³âL¯ð?©¨¤j×/?Š¾ZÄÎ=?îeu¹{È_?Š¾ZÄÎ=?—ë¡ûG&?¢t(ºÂÞ?ï@¢÷³¢§?¢t(ºÂÞ?ÃŠ/£™"?©ßÈóêÂ?ï€ñ×j¬é?©ßÈóêÂ?Õ¿™4¼A²?·
×ߌ?å 3e¡ß'?·
×ߌ?p\Òß±?^ø©f­É?ïßGüC?^ø©f­ÉPSR3FGL J0937.7+5008@dëÿ´€¦@Gbž À:' €©ÌÀ;ömÏç3€À!͋¹‡ @8e>É…@äÀ^g¿â¯îyèÓ¿ç'Ã&l¨¿åîÏÜÕ60¿à¡xhÐAGNfsrq@'1cø¶PowerLawGB6 J0937+5008?ïõÖʍ¾€? .D$áЄ?TRjçB¯~? .D$áЄ?ïäÆ\ßî¬?€î}DÐô¸?k9£>Mãw?€î}DÐô¸?î½n£©?œbXú<þ€?¤/‰>¡n?œbXú<þ€?ð=À'0¶š´='*"UɬD=À'0"¥/6?ïøÙ-l—?X盝'^)?L›KPFëð?X盝'^)?ïn¯Ìœó?¦º¦¨¢€[?'*€ûý?¦º¦¨¢€[?5@»?ÒŒžAE±?¦.,«ôT?ÒŒžAE±?ïÿÿþc®â>Uòtl")/>-J"a÷¿>Uòtl")/AGN3FGL J1031.0+7440@`ǗͅY@CšÀ ýÀ:&sÔ
2îÀ;´¦ÏB.À!͋¹‡ @M†ÇÚʑ@,"ß}ÿ_¿ÎY 
ý¿ç¥b•ÿä°¿Ü[z"0t¿äSr€'TAGNbcu@¨‡†)ñkPowerLawS5 1027+74?ïö"f
O? .OY­ö?RÙ3î³;? .OY­ö?ïä×$`ÿÂ?€éEiÆ·?k(Û¬¾®_?€éEiÆ·?ïÓªŒ†?•ÙÞqÿˆ?žŠ®o>§?•ÙÞqÿˆ?ð=ÚÃÇöòª= ÚØË
d£=ÚÃÇ
Ô_?ïû(žôf3?RQûÉÝ(?C]"ÞS4i?RQûÉÝ(?ïcÁ®5²ê?¦ÿ"ÁºáB?"‡Ê@(Ú­?¦ÿ"ÁºáB?î»°l'E/?›­B¹{Ú?¤Dù9b?›­B¹{Ú?ïÿÿýÚ>ƒ>W¯¾Ãƒ³>0àk:8>W¯¾Ãƒ³AGN3FGL J1159.6-0723@q'Êßø"¼@J¢€dÀ9Ҙ×ÒºMÀ;¢Òhî#À!͋¹‡ @x†ä'@Ôɀ'±¿æQ:›:G¿Ør‰ñ¹t¿æð±$´|¿¯ƒ-–mžAGNbcu@ Ê €sWæPowerLawPMN J1159-0723?ï»2—ÆŸ{?°êréÆF?3Yÿ'ÏX?°êréÆF?ïátà¸Î#?-U'|t?n‹‡Ê"1?-U'|t?î­ãé|Žz?›x:uÞÉ?¥!ÁfJj?›x:uÞÉ?ð=º{¶$»=‰u,#¦jK=º{šk˜?ï²úüé}»?–ïàó×Dù?ƒA@·â!K?–ïàó×Dù?ïdºϪ<?¥£´ÚЌ?"h½ ãN"?¥£´ÚЌ?íËø¥¦‡?¡Æö¹?± ?¦F?¡Æö¹?ïÿÿýÚ>ƒ>]øt‡³->.Ó(Ö°Û>]øt‡³-AGN3FGL J1832.4-5659@u#–Óõ¶À4¯ÿ6¬dÀ9>ô×­Ñ_À;–Ë1ÂëÀ!͋¹‡ @´:¹ºKk@'¾Ÿã_¶¿é!á+ ±¿Ù
¨4¼ö¿è­·ŸOLU¿â.e-"ÅIAGNbll@Ža=æOUPowerLawPMN J1832-5659?í[̕«‰—?Ë~©³¡?µ!›S¦Å?Ë~©³¡?ïÑ|‰éMa?‡îã= ¡*?wA»YO}?‡îã= ¡*?í³Ÿ·h'?¢Û}ç!çÐ?²cHx¢{?¢Û}ç!çÐ?ð=àå»þå	=ª},ÂÜX=àå»þå	?ìlP¯ŽŠ?Áû.uçÁ?¼úƒ‹³?Áû.uçÁ?îÌl ©\Ÿ?´:©³2ô?£9=öF?´:©³2ô?ë¡Æ¿«¾?©ÅÎ/<Gs?Áxå¥Q?©ÅÎ/<Gs?ïÿÿùK*>s Ùëôz>KçßÏ+>s ÙëôzAGN3FGL J2358.3-2853@5H€_5ð}ÀSŠ« ,ZÒÀ:GpJ붝À;õxZ"±À!͋¹‡ @žIaÈÈ@OãÀYK÷¿ßÐ¥æ?JÕ¿ê®tŒóe¿ÊTLªË¿ïÿ'£+ÓAGNbcu@ŽOù¿ß~€PowerLawPMN J2358-2853?ïñd€L? 0±L"B?]6ÿ0ýAí? 0±L"B?ïßbDSþ?…3&·¾Œ‡?pNÝÜà-a?…3&·¾Œ‡?í}N»¶
O?¢]®èÕ$?´Š!áº
?¢]®èÕ$?ð=Üéáú'»d= %ÏîÑ=Üéáú'»d?ïù¤¼bqd?bÚd?8²Ì?Im†+Ò?bÚd?8²Ì?ïŒaÁÕ¼¤? ŒJ§Œ+?ŒçŠÖì? ŒJ§Œ+?î2´nï¼? ¾ùuÏ?¬Ô¾}OI? ¾ùuÏ?ïÿÿÿv¡>8ÀnØ?Òá>[›‡kj>8ÀnØ?ÒáAGN3FGL J0534.5+2201i@g´ßݵÀö@8ªAÀ5¨†¡oPñÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ú=p¡'Øa¿Ó×o9ìh¿Ù3Ší•€l¿ÍÉB˜o¼À¿ÍЁ~+^OTHERPWN@@PowerLawCrab?ìÃë$%Ï?È"rTÊ÷N?¹à¦Þч?È"rTÊ÷N?¢wCÿdê?ÁMÚuÏ1?î؋ÀE³q?ÁMÚuÏ1?éJǬY?±Ô­Òò¼Ý?ÊÔã«¥N?±Ô­Òò¼Ý?h"tϨNß?¬U£]å?ïçl‹C•?¬U£]å?î(ÿ§ÿ?º£­ÈêXé?­p÷7Ü?º£­ÈêXé?•
4…"‰Q?º—å(Rs?ïW–[îà•?º—å(Rs?íFºoZ´_?¦gèåÄâ?µÊ,ƒà'‰?¦gèåÄâ?`bMÒñ©ü?¦ßÚwƒÚ?ï-V?¦ßÚwƒÚMIXED3FGL J0833.1-4511e@puR}ÔAÀØðߦ™1À6!vu¨"ÉÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@G̀&¿äqªé3q¿æe¥åþ™¿äqªí~óü¿ä§ÍP¢§,OTHERPWN@@PowerLawVela X?ëßÖ0ñ	?˟4Xw:t?À€§<;çÚ?˟4Xw:t?¤Ž*Woè?'0=×ÉM?î·Z{C?'0=×ÉM?繘ی5á?±ÓUK7Á?ЌÎHç"=?±ÓUK7Á?h"tý& ?¬U£]å?ïçl‹C•?¬U£]å?캿GíÄ-?ÅÈ´º1j?º*À'Þ˜?ÅÈ´º1j?˜:.‹??¼jš8â?ï?ÇéÓv?¼jš8â?ëPֆ"Þ?«a研ˆÙ?¼¥çt‡«?«a研ˆÙ?`bMÒñ©ü?¦ßÚwƒÚ?ï-V?¦ßÚwƒÚMIXED3FGL J1514.0-5915e@tQ¿zÔ²¿ôWõÀjÀ7Ï{-ÇýÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ù$5½À¿Ñn£ Öå¿×!ƒït~¿Ñn¶t¤J¿Ð…[/aӖOTHERPWN@@PowerLawMSH 15-52?ë*†ãƆ?Ì´D'e©¹?ÃUçàpåé?Ì´D'e©¹?¦öµ8Š?Ã{\Õ÷vw?¬cº~?Ã{\Õ÷vw?éå†7Uñ?±b9y[?Èkç"¨:?±b9y[?h"u	a¾?¬U£]å?ïçlŠº%"?¬U£]å?í0§}Ì£?Â&
OS<?¶ÊÅ[ud?Â&
OS<?™×"®Y-é?¼ÜH2ý5ÿ?ï1Fꨳq?¼ÜH2ý5ÿ?íFË͸?¦¹tVCL"?µÉ¡'­h?¦¹tVCL"?`bMÒñ©ü?¦ßÚwƒÚ?ï-V?¦ßÚwƒÚMIXED3FGL J2021.0+4031e@Sp¿ñ7@'˜à66À92šs´-Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?øzá? ~æ¿Ð&
ŒT¸¿Õ¨xöræ¿Ð&
±Õ‹É¿¾pç&räOTHERSNR@@PowerLawGamma Cygni?ìüâo)E?DŽ-"-'?¸쇓ŒÙ?DŽ-"-'?¡ãfñj¿?¿^Vø_LÂ?îáɐ¤ŸÔ?¿^Vø_LÂ?ê(·hÙՖ?²³8Òße?Ç]"\˜©§?²³8Òße?h"vÈô#?¬Uëè?ïçl‰Ô?¬Uëè?fŽ÷¢?¶6d
ه?§…é—…è?¶6d
ه?–#¸e
€?»mԓ?ïO&âJ–?»mԓ?ììVyx+?©þÙĔàp?¹âL4>ª?©þÙĔàp?`bMÒñ©ü?¦ßÚwƒÚ?ï-V?¦ßÚwƒÚMIXED3FGL J2028.6+4110e@Sæy€žQ?öVŽà3·À5$‹
Š}Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@ff_°iÀ¿á¸•Ý0r¿ãêáF›3¼¿Ê²ôQ©ž}¿ãÊ­" ®¡OTHERSFR@@PowerLawCygnus Cocoon?í$¢Öüã?Ç'‹6vÖî?¶Úï2ÿæè?Ç'‹6vÖî?¢»{?=?¿}2/Óo?îßHuJì?¿}2/Óo?è¡y	ß°]?±j:s}×ð?Íz؁>?±j:s}×ð?h"tÑ&Ý?¬U£]å?ïçl‹C•?¬U£]å?î»´wkq?µX¬q;P?¤N"»øäå?µX¬q;P?—¬{&D•å?¼œ£
ëe?ïBœ'"€?¼œ£
ëe?ìÚ"2¯Õ›?§-‹de?¹.îk]:&?§-‹de?`bMÒñ©ü?¦ßÚwƒÚ?ï-V?¦ßÚwƒÚMIXED3FGL J1513.9-5908@t#àz(»¿ò—™:À7Ó%ô†O:À9ø˜˜—;À!͋¹‡ @d<˜â'@óƒÀig"¿ìÆ¿u)¿ìž=e^¿áÃn/Ĥñ¿ÒºTûPSRPSR@hÏ×6&-PowerLawPSR J1513-5908?ÒI玳ÑB?Ò‡M€€2?æÛ8¦_?Ò‡M€€2?ïÀïQJ?Àöµ‰?ˆW6тÿ?Àöµ‰?àÓ+‹Áa?µù!µ"Ç?ÞYÁ¨è}>?µù!µ"Ç?ð=£wN‹K]=g0‹37=£wNX¿¸ž?àn
)¼Åv?ÒL`"Kü¥?ß#嬆u?ÒL`"Kü¥?îP¦ ­Ï?¹9™dü•#?ªõŸç¬ñ?¹9™dü•#?æ–f֛?¶'¦µwJÙ?ÓéÒÓ2RÊ?¶'¦µwJÙ?ð=÷€ä^W¥=Ó%˜?Ú>¥=÷€ä_¦}'MIXED3FGL J0121.8-3917@qU{à~íÀSË¿ñò÷À:¾8äMÀ;ÿÍ2MZ&À!͋¹‡ @èw9@?üÊb&%Ú?ïôöŽ®¿á°ãôAí¿âO²vE'¿ã2ã#žUNASNone@³×Kà7ÝPowerLaw?ïö"¤ŒK? .A›¬Í?Rö¶©jŠ? .A›¬Í?ïÛ¶FÎq?‡ûZ&<?ry¤àc³?‡ûZ&<?îÒ7wæk"?—Éô塃>?¢Üˆ",ü·?—Éô塃>?ð=ÆÇ]L£Ål='V«†àÙj=ÆÇ]G­?ïýá:]?CÝRЈ?0÷9*)?CÝRЈ?ïe܃#5?«Ü8ù¼\?"Do À¸?«Ü8ù¼\?î>P6æ? '5ï"?¯Ìü(Ü¢? '5ï"?ïÿÿþíA>HÇ*é¨âo> >¿—qÎæ>HÇ*é¨âoAGN3FGL J1655.1-3954@u',à2Û@ÿ8x[0À:fÿš6À;â1¸ß°À!͋¹‡ @;,‡óSõ?úàåáâ"?ìºvçpš¥¿çIÕ·¿ÔuÌX2¿ã'?™UNASNone@ÐTOß;dZPowerLaw?ïÕ$*	qv?ªâ½*ìˆl?umëÓè ?ªâ½*ìˆl?ïÁ³Øµ
?–[vžAõ?{¦g©f?–[vžAõ?îÇ
	Ä?¡eî^ñ<?®S,ÚÞÆ?¡eî^ñ<?ð=ÿ˜Ýk­©…=¼cŒá(¼=ÿ˜Ýj†ƒ¨?ïåLW¡Á?‡µÆ'm}?j³ùÒùf{?‡µÆ'm}?îÐiÜ´ï?¶ÄŽÌ-å?¨ùb4±?¶ÄŽÌ-å?íÀï7Ë?­:ÁÐx©?·ôú>©?­:ÁÐx©?ïÿÿüÇ]Ä>a0³'µ{>8oƒcğ>a0³'µ{AGN

==> SOM_VIZIER/3FGL_prob_catalog_2classes_SMOTE <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  274 / width of table in bytes                        NAXIS2  =                 3034 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   33 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\SMOTE\3FGL_prob_cat...'TTYPE1  = 'Source_Name_3FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON    '           / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Signif_Curve)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'ln(Variability_Index)' / label for column 7                          TFORM7  = 'D       '           / format for column 7                            TTYPE8  = '500MeV_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'HR12    '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'HR23    '           / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'HR34    '           / label for column 11                            TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR45    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'Category_3FGL'      / label for column 13                            TFORM13 = '5A      '           / format for column 13                           TTYPE14 = 'CLASS_3FGL'         / label for column 14                            TFORM14 = '5A      '           / format for column 14                           TTYPE15 = 'ASSOC1  '           / label for column 15                            TFORM15 = '26A     '           / format for column 15                           TTYPE16 = 'Flags_3FGL'         / label for column 16                            TFORM16 = 'I       '           / format for column 16                           TTYPE17 = 'Missing_Values_Flag' / label for column 17                           TFORM17 = 'I       '           / format for column 17                           TTYPE18 = 'AGN_BDT_S'          / label for column 18                            TFORM18 = 'D       '           / format for column 18                           TTYPE19 = 'AGN_BDT_STD_S'      / label for column 19                            TFORM19 = 'D       '           / format for column 19                           TTYPE20 = 'PSR_BDT_S'          / label for column 20                            TFORM20 = 'D       '           / format for column 20                           TTYPE21 = 'PSR_BDT_STD_S'      / label for column 21                            TFORM21 = 'D       '           / format for column 21                           TTYPE22 = 'AGN_NN_S'           / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_NN_STD_S'       / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'PSR_NN_S'           / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_NN_STD_S'       / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'AGN_RF_S'           / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'AGN_RF_STD_S'       / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'PSR_RF_S'           / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'PSR_RF_STD_S'       / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_LR_S'           / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'AGN_LR_STD_S'       / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_LR_S'           / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'PSR_LR_STD_S'       / label for column 33                            TFORM33 = 'D       '           / format for column 33                           DATE-HDU= '2022-01-29T22:25:37' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             3FGL J0001.0+6314@]RÂÀð ?íŸWÿÎàVÀ9ZzŸÙOÀ:ÿ!Z³¿õÆkvñxÿ@Å "	¸@ܾßú&!¿ç0WìPӿ쳊Ügu¿ÜƒûÂكê¿îæý/k'–OTHERspp?/w?­\¶á>ú¥?¦æÏN]"?­\¶á>ú¦?ëÖ#¾)ãá?ÏàʆÆ×?À§qXpy?ÏàʆÆ×?êk«R,U?°Á—
¬×?ÆQQ·N¨?°Á—
¬×?ï÷­L^v{?X šœçÒ?P¥gCR?X šœçÑ3FGL J0001.2-0748@VAk¿×ÀPÔÀ€"ÐÀ9"ñóÍÃÀ;¯Þ>Xˆ?ä‹|¸&;@Avû	 @1݀#Pè¿ÔÇZö#eé¿ã+ùÖζå¿Û5šÜdÅR¿í›Q÷æÎAGNbllPMN J0001-0746?岃k¤¬6?ÆQ+Ⱦ"?Ԛù(¶§"?ÆQ+Ⱦ•?íòœZŠ/?·=&±%?°k+¯.‰?·=&±%?åÆ®JBmâ?·_lZæ?Ôr£k{$=?·_lZæ?ê	õèõ¡£?±É	¤UU?ÇØ(\)yp?±É	¤UU3FGL J0001.4+2120@Zê–_RuïÀD	@¢CÀ9‹!P²ŸûÀ;ÎÑPÀô?÷ÁF#zÙe@{J¨š¾@d´¢´uh¿ã©OºÛç%¿êJJAuHà¿ïÿ:ÕÇ?º{	¥_rAGNfsrqTXS 2358+209?ïÿ…NÇ0k?:M'?¬N3å>-?:M'?ïî˜Åΰ?h!óX䶖?ag:æ1OK?h!óX䶎?î¿7Iœ¸m?š~Á€P²½?¤‹f4y??š~Á€P²½?ïaŒè†Ã?¤h%.íL?ž3Îbï'®?¤h%.íL3FGL J0002.2-4152@tá !¸ÀR	"`¸À:†¾š§·À<˜¡L'¿ùº­ Œ§ï@ \2°@¶ÆCò¿éÖ%8ý*@¿çž>éí‡?±Dņ YÖ¿â"yq…ÿ3AGNbcu1RXS J000135.5-415519?ïÿæŽû B>ìêá…\²s>éqß¾(Æ>ìêá…\®è?ï÷_"øž"?`Ñc–hÈt?Q@ÖÂÛ?`Ñc–hÈo?ïäÆšl?sL†ØT}›?k~9e"÷«?sL†ØT}•?ïÿö½`Ü>àÌ)§#>Óè…>H(…>àÌ)¥¹3FGL J0003.2-5246@sïž?»×²ÀOiÿ¼ä!À:‡¯»DMÀ;èK	éÎ¿¸otpl@€Ä©Ü¡?þRÅ؈B¿ïýñ$yœ?ﶰÅýr)¿ÙjÓ³'	¿Ý¾_îõcAGNbcuRBS 0006?ïÿ:µÎ½É?Æœ¤à?©F(GG?Æœ¥µ?ïòM þ1Î?e1M@\õK?[e¾œc®?e1M@\õO?ïÈqöàIÕ?yw©PèbD?{ǏÛJ?yw©PèbJ?ï×]¤É׿?nD	8–Š?tQ-›è?nD	8–‹3FGL J0003.8-1151@U¤ YÀQÅcÿï9À:¬"V;uøÀ;ù è­Óã?âŸ8ÅCk@
¢'<@0+ÿ>l?éyÑyý‰¿ØóK^¿åD:Ï<q¿Ü¼ûßðýAGNbcuPMN J0004-1148?ïƒéB4PÌ?›© âW÷?¯rëÍV?›© âWö?ïé÷ÿ-?w&P:È•?fø÷Ós?w&P:È—?ìùäCi&Þ?­D}ï®	?¸0Ýä¶É?­D}ï®?î€W|yý`?"'¢_ÁH?§úˆ8`)þ?"'¢_ÁI3FGL J0004.7-4740@t=Ÿ¶MÀPá1ÔÌvÀ9iÎ,H]gÀ;؂—õT«?ãqP7®u§@è<Vžó@:f¿§ C¿áMwé+ä¿æXÜZ½³¿äXzLnºë¿ïÿð¸å9UAGNfsrqPKS 0002-478?ïýúS­o?6ü|lÙ×É?0-b—T€õ?6ü|lÙ×Ç?ïÈQ«PþŒ?ŒMq4F?{×*W€¹"?ŒMq4B?îr@ ,›W?œ$"¼AÔ?¨Ûýý6J'?œ$"¼AÒ?îÆ*é?"ã?qE«q?£ž®­XR?"ã?qE«r3FGL J0006.4+3825@\U=žÇÀ7‹@;À9Jn¿Ñ;ÇÀ;™2"Ѽ?êXyç¼V@&í @ïဎæ¿çGkÚ¢+¿æÝH
1ÿìNC–œ}é¿äz"&V½AGNfsrqS4 0003+38?ïûPãƒé1?AOùçÚτ?B¼qð[:N?AOùçÚÏ~?ï>·Õ¶
Ù?«™8=íÔ?˜)I>Dô?«™8=íÓ?ïQËâÙ&á?Œÿ†'µÔ?•Æƒ¤Û#Ù?Œÿ†'µ×?ìÎÛÝp¥?°­¢ðås.?¿Y‰!z×?°­¢ðås.3FGL J0007.0+7302@]ê_á'p@$ëÎ ‰ãCÀ5"á÷|þÀ:H!ß&¡@ö%/Íù@¨Œá¥Kÿ?øè!¼é)û¿É_:@KRA¿ÙyB+s¡7¿à掝¿êwë1olRPSRPSRLAT PSR J0007+7303?o|>‹Û›?"R+F¬ú?ïàƒÁt$e?"R+F¬ú?eÝãYm?€Ô"~"n?ïêø"<\§?€Ô"~"n?F5ŠK£8? 1#§øtÝ?ïÎS­¢è? 1#§øtÜ>þ¶^| ›?ª°8Čä?ïÿ"CÆ?ª°8Čå3FGL J0008.0+4713@\ÕH˒:À.WÊÆbÀ8‹e²€gÀ;<µgUy¯?íñvi,®@Ó=…Ï@+?ëÓM¿ÀvþF
ø³¿àœ €Ò[¿Ú̀èYˆ¿äC9qzAGNbllMG4 J000800+4712?æ´3öD‡³?Æ®®¥Pžõ?җ˜vð™?Æ®®¥Pžõ?Ɔ1Ï/\?Ìî©t\®Â?ê^s¾Ì4)?Ìî©t\®Â?ëLwÎMú?ª³dÈ?ÂÎ ÆÈÀ?ª³dÈ?ÍÄâû?±R²!¶?èŽýÇ|>?±R²!¶3FGL J0008.6-2340@I#ڿԖÆÀSð*ùš‹À:c)ÒaaDÀ;¯S;ç6Û¿Äû¢£-—@ÜAƆb?ù•<@5? °ò?'Õ?ïüz¨£Þӿ窜>öœ?Ú£¤6¢ö²AGNbllRBS 0016?ïî{ nž·?c)|c$ý?a"ß'aG}?c)|c$ü?ïô$\>ž?cto"sj?W¶áG'¿Û?cto"sf?í»:Tæ?¡üÉÜŵ?²&/-XÏ7?¡üÉÜÅ´?ïú¢?K§†Wi…ì?EwŸ™Ëö£?K§†Wi†3FGL J0009.1+0630@ZMa²¢ÀKlR@>´qÀ9Íêï̓À;µþÓ°Ý¿ïæJ˪@w"²î'@oV@S'3¿àmíóQá¿ã-˜û¿áW¹aÏÿàŒ*h¼àyAGNbllCRATES J000903.95+062821.5?ïþ'{
«?'êäp#Û?&߈O%UJ?'êäp#J?ïôIcóO\?b#Él\ä<?Wm8aGj?b#Él\ä:?ïy‹óí3v?‡ñ=
i?Î'Y'<?‡ñ=
j?ïýÁÉ[…?.óÍyœÖ?1ñµ#׆ë?.óÍyœÖj3FGL J0009.3+5030@]s`Iì³À'›I ÛAÛÀ8ҍÖí¸À:ú€ÌC:?èNêj±="@e鋁 ?þÛ°àˆŽ¿á"¢x1¿Þ&úÓùÅ\¿Ù͹"¤³¿âQ®Ñí§AGNbllNVSS J000922+503028?ïþfþóÅÏ?,«ÒAáOÊ?)ã
*?,«ÒAáOn?ïQ¾F7@Ò? Á'h²¸?•È79å¤? Á'h²·?ïyf… K?‹—ŸªDG?Ó/NKö"?‹—ŸªDJ?îŸâã`žØ?"'øžÒh?¦ÑÉöž?"'øžÒh3FGL J0009.6-3211?ôÒÆ>¾ÀS愠
Q!À:iÁµA•ÍÀ<YQªí?›¹ÉŽ©H@™ÎØÿ@zSŸd^Ͽ〠ƒ¿ãô](5dw¿æ¶"Ò
¿äbzª¨hAGNbcuIC 1531?ïèŠk?rûÊÀ=ž?gàó÷u–	?rûÊÀ=Ÿ?ïêå	ÌÇ?pŽ
º4?ebö38û?pŽ
º7?ñŸDÑ?™®hõ¸¬
?¥÷àæ²ñ?™®hõ¸¬?ï(‡ˆP¤?‹'õ)f*?šïÿëf?‹'õ)f*3FGL J0012.4+7040@]ëþ?5Ÿõ@ Ì <ÁÀ9Ê ™ÙZÀ;KÀæå|Ç¿ù¦®ÕëÚ@‹`Þj.@Þ¸@xÁ¿ã
Q2L®¿ëÓP¹?
¿â1Àª³%¿ÜGÐç—1AGNbcuTXS 0008+704?ïÿŸðµ£(?v)‰tþ?җ5®?v)‰uá?ïÕ)cƒÉ?‡,zsõ¹š?ukN>?#?‡,zsõ¹›?ï¹%ºbÓo?~‹Æ­t?¶'gK$2?~‹Æ­r?ïÿ–1 Ã? ¹¿Ÿu?
`3·Ï]? ¹¿õ3FGL J0013.2-3954@tÅ.@…+NÀR½"@(äüÀ9¯ó¢#«×À;ÛÞ|!¹Ž¿þ)
Ðx(@¿(Ÿ[z@±»€Hj¿â4¨©,	¿ä+P)§Þ¿â¹).<¿Ös³Èç1tAGNbllPKS 0010-401?ïÿX*õ…ì?!íÙøs)?ú¡OBf ?!íÙøs:?ïö_}î]ˆ?aë]QI·K?SA#Dð¶?aë]QI·M?ï¿´ÓÒÿ¡?€š-W¦ø?€Ë@Æ?€š-W¦û?ïÿÖ۔lí>ùL®;¾F…>ô'5Ɉê>>ùL®;¾K"3FGL J0013.9-1853@R¨øäÀS…€,á
À:¢ÐqœûNÀ;þ¦Ë±CÚ?ß!0wþ$š@Äû—»s?þö`¾ø?ïøÀá\%ñ?Õæ/–½é|¿ÚëlÌVo¿êǦ—}"AGNbllRBS 0030?î¾$Ú½¦?¬× šD?¤²T'©?¬× šD?í,¶ûïçE?ÁåQA§p?¶šH €Å×?ÁåQA§p?ê|XÍ4'¤?°U&K"%?ÆœË-¹m?°U&K"% ?ë÷gcÖÀ?°ÎUWw±á?À"bs¬¤þ?°ÎUWw±à3FGL J0014.0-5025@s×7À*ýÛÀPh"  0øÀ:™û3èdÙÀ<0{ÈÎ;?×Ɵw»3®@±Ëžðñ?þÈ3€5'¿ç§vóÁ.¿ÑÔ'54P{¿ä/çP~$¿ÜºhÆïƒAGNbllRBS 0032?ïëW(<?qs],pÿ°?d¨×êÃìÊ?qs],pÿ¯?ïè\¥ ñþ?t,%"1l?g£Z߇?t,%"1i?ï¬nÝ*ð?—À»>¸Â?Ÿ
r$Z¡Ù?—À»>¸Á?îØ_^zJ·?"ZÕ*Kĉ?¢z
[T•?"ZÕ*KĈ3FGL J0014.6+6119@]¡ñ'l¿óÑ=ŸÈ²·À9"=ëóفÀ;QÙ($â8?ìqÌ[ã¬@k¾vçÂ?þ3#Þ¬s;?î'NË®Ùa¿µ™^'Ÿ"¿ÑÃñ)è ¿ÝWGph.#AGNbcu4C +60.01?ïÈù]‹âL?~ë(•/ò6?{ƒQ:Úu?~ë(•/ò5?âÀ8È:®?םï}?ÚӎoŠ£?םï}?)'Š?—NèS~Ž®?¥uߝg×s?—NèS~Ž¬?îeœéµ¾?›l¶×‰šL?®)¦1d¤2?›l¶×‰šK3FGL J0014.7+5802@]"Ñ_ÄÖÀîQ`Dä6À:.[)òBÀ;'Y5%{»¿ÙN´þúÇ\@
i•ûg¿?þšåŸ¶´?퐗Ã^B?ꎽ¢ãD]¿á>Ö¿áA"HŸkAGNbll1RXS J001442.2+580201?ïò¦j?a»Ó¬Âò?[Ò³ßõ+ý?a»Ó¬Âî?îAÇ1'¯a?·º`²Yµž?«ãŒæå	â?·º`²Yµž?ï*ʊØz?ÞÊKy¥?š¦®½"ð¬?ÞÊKy¤?ï«Ÿrš?†·7™Ý?…9˜<cY»?†·7™Û3FGL J0015.7+5552@]z,¾¤ëÝÀ˜>àŸ°À:])¦ÂwÀ;§UCÿ3?¥¼RX‹‰@

a'Ñ×@êÀ/¿ã•ÖÞ¾¿æ®ëFÏ6"¿âªƒ&:§F¿âÓ´`ÖjÁAGNbcuGB6 J0015+5551?ï÷F±U¾?TíF«Šï^?QÏrTƒB?TíF«Šïc?í?ß=`®?ÀXûKPÕ?¶úä?ÀXûKPÕ?ï­Ý"gÊó?€CÒ
ááp?"ˆ›&
Cs?€CÒ
ááq?î˜Q,Áô_?•pHÃK‹?¦zí3àº?•pHÃK‹3FGL J0016.3-0013@ZáuÑ=ÀNç…`&±EÀ9;ŸDÔEgÀ;¶QºÝ·?ó¢xËmÒ@±vÚý½@ñ]À¥w¿ã¼²Læ/¿éq`œfÂF¿í¨Âñ¤¿ÖÆQ÷!<ÄAGNfsrqS3 0013-00?ïþôÜÞ?(TIêâš? ¾²2,¾?(TIêâÈ?ïðNM=ï?iq<Ž:w?_ce…ø"º?iq<Ž:{?ï:ó1Mr‹?üfCgdˆ?˜¡™ÖQ®€?üfCgdˆ?ïË!¿!ê?˜¥.'¡¯Ø?F›È¦?˜¥.'¡¯Ø3FGL J0017.2-0643@XêÉ`0Â@ÀQSÙÔóÀ:*V]çÀ;Ï% £y¿«NÐÅMŽ@øœJNì@íø@˜÷]? R
Œçã¿ÅrdgnàD¿æhuµ8Ü¿è¯4Ã×ßAGNbcuPMN J0017-0650?RFE? ¥"÷3iÌ?LNÕ·7i? ¥"÷3iÌ?ï'WH(¼P?˜Çwç,?‹ª-õÐì?˜Çwç,?ìɬIþ?©Ö^u;¾=?¿!²±â?©Ö^u;¾??î!ŠëV?ž‹:(5™?¯Þ=çQJ©?ž‹:(5™3FGL J0017.6-0512@YPŠŸb0ÀP©&¿òÉ·À9)´xB0ýÀ;cî4üa?ãÂÇàÔÁŽ@Àù™´qŒ@áÀ#ñø¿äÜEZ…»¿æéú`"üb¿êvºÏý·¿àÏÀÙ5AGNFSRQPMN J0017-0512?ïÿHK¸f~?ìž\P'‡?öˆó0BE?ìž\P'¡?ïô9ªÜKB?d¤Ümˆ/"?WŒªGiy–?d¤Ümˆ/?ïqø{?‡Øð>4Y8?'ÀðœÝ>s?‡Øð>4Y9?ïü¸eˆ?6ŒÁêç'?:;|Ó¿?6ŒÁêç¢3FGL J0018.4+2947@\›¨d©ÎÀ@Dߥ¥À:´Ÿê$ÌÀ;ú"#—µÀqÌMËåÇ@r÷na?ýÕ
ÁÉR?ìQ+êr,Ì¿êàƒKà^¿ÅAí§"¼¿Æ(·±TÒAGNbllRBS 0042?ïÿél¥¶>ñvnܠƳ>æü"ZI^`>ñvnÜ Ãó?ïïë@žÃ?m÷3µ	ü?`í¿a='?m÷3µ	þ?ïÁ!×?'ŧúòÌþ?{ïvy"í?'ŧúòÍ?ïÿÿ±R»>™€è9Ô£%>‹Ó«QEbç>™€è9Ó§¦3FGL J0018.9-8152@sH _ñØÀA"á@!X?À9¦8‰´IHÀ;©‹K"=B¿ò½¡ÜF@ÍnkB™@š€ ¤OÖ¿å¤püÜ#¿å¡g÷¾œ¿à–hjU;ú¿Ñw-HrAGNbllPMN J0019-8152?ïÿéû°Ú>çd
nEä>æOb(j>çd
nFÙ?ïï¾Þ{;Û?khõwt	?`A!"Ä#æ?khõwt	?ïî~¬UÌ?hBœt%ná?aSª€3ß?hBœt%nÐ?ïÿˎCu>úïÕ¬éa2>ú8ÿ^Eƒ«>úïÕ¬éa*3FGL J0019.1-5645@s{´?¢­?ÀMéE¿ý±qÀ:OÁä;~[À<mùÞý¿ä ìî¥{@;N	Î5@  €´ã¿ì;—"°BA¿Þ݊t¸Ž§¿ã'L]"H,¿ÑçeÈdeäAGNbcuPMN J0019-5641?ïü6b>"ç?Eúj`½AT?>LîXÀm?Eúj`½A\?ïó¥üŸ×"?e¯sð2¸?X´ÀQ¼2?e¯sð2¸?ïN/Ö
Ýí?""É\ˆ?–:>¤Bu?""É\ˆ?ïý«êc–?/Fü‰'É?2 ¬ç;PZ?/Fü‰'s3FGL J0019.4+2021@\5ý~E€=ÀDð[ÿÛÀ:dZUÖÀ;ã]9–û¿áÕå
C@ñxô@ý1 6ç?ÚHtŸ|¿ë¢CgÄñr¿ÚESÔ	úL¿àû7Ê$Y"AGNbllPKS 0017+200?ïÿä92§Í>òtI#èV>ëÆÍX2¨£>òtI#ço?ïð¶/%ó?e	×Ζ¶G?^" å´¾?e	×Ζ¶I?ï­v¿­Å?ž6õEØ?"¢P»Î¨?ž6õEÙ?ïýbw¥µÌ?.©IÝ}8?4ìBÒQ ¨?.©IÝ}p3FGL J0021.6-6835@s01€
|[ÀH&a_–hÀ:J¾ò¶°À;ÿBûÅ¿â~Ž,öOŸ@–CPŒµ[@8B«v'¿äé©Cõg¿èÏÎ@F¿çú˜ž-8Y¿ïÿPÓP¹AGNbcuPKS 0021-686?ïþSU¿¤?5BâL¬?.úʤºš?5BâL—?ïÞüòN`?xف2'àQ?p†øXÏÎ?xف2'àS?ïtymfN0?"švvîŽ?'pÒS6:?"švvîŽ?ï½Hé~‰?wq܏R‹?€­Å ]¸W?wq܏Rˆ3FGL J0021.6-2553@Dçڟô&®ÀTÎ]?á—_À9¼º"eÀ;Ζ67Ê¿ûõõuã\@$|>M@ËVß_Ìn¿å<RÐÝS¿Þ®îñËðë¿ÜR¤J«'"¿ã>"¤âD{AGNbllCRATES J002132.55-255049.3?ïÿ6	‰0'?GØÓH?>ÎÙí»¥?GØÔ?ïõk3q
?cmyÊàE?UÁ)™èg?cmyÊàF?ïÖ<¶Þ±?ya3YçT?tᤐü¦¥?ya3YçV?ïÿÕö=A.>þè\uínç>õá_h{§>þè\uípÒ3FGL J0022.1-1855@Tû_ò®ßÀSØÊërªÀ98?±Æ·	À;NQ"GJA?ìˆÓY'Ž@ÞÊÏÇ~?üÈÇ>Ã_;?î¯ÎE.¨¿Ø.¬Ï¿ÐìBÅÿ坚ݼ^@AGNbll1RXS J002209.2-185333?ïû½2Œw ?@æR¯³ý?A5Î!{t?@æR¯³ë?ïáô(¶½?v"íA"?nr×IBñ?v"íA•?ï8	%ôÍ?'.€©?˜þÛAf\}?'.€©
?îÛF}Aøæ?•ÉeÊK?¢K˜+àqˆ?•ÉeÊK3FGL J0022.1-5141@s™ìºËCÀP4߀-·ÉÀ9'컝oÀ;®,nóÓ¢?áDÂé–~@Vál)?ÿ̅>õ!?Ô.¢)àú¿ÙݪƐ¿æR¢¢Ša¡¿Ð0žú'¾ðAGNbll1RXS J002159.2-514028?ï×õoò?u¢g%ÆU?tH¸z¬?u¢g%ÆT?ïð(8b_‹?if'÷nó?_¯;@êñ?if'÷nñ?í"+\Wì?¤f{µ.ˆ¯?³Þ¥@ŸÚ?¤f{µ.ˆ®?ïL6vŒû¨?Ž¡Ô.8í?–y1.`Šß?Ž¡Ô.8ë3FGL J0022.5+0608@['¾‹ÁjÀL V·À8s¹NjÇÀ;:ÑY#‡Å?ì½Ã²œÊÑ@9aÜ>ò@–_¡PG¿Øÿçƒ~Ç~¿âœ§jŠò¿àjT7˜PL¿ãi,¶0BAGNbllPKS 0019+058?ïÿaTù?&Ĭ'[?Üõ}@Ãl?&Ĭ'<?ïÞGÃº>?t€ÒÌn2-?pÜ?"áV?t€ÒÌn2+?ïOÞý5?';)akD?–< Y_­?';)akD
?íҊ4:Âö?œ™S!®}?±k®^)èW?œ™S!®}3FGL J0023.4+0923@[Ý? §?ÀJmÎÿ¬óéÀ9¥:¿ïn¸À;×Ájî‹?ûðT5:Ÿ@ƒ`–mÀ"?øbÀú†™b?µ±¬lÒ]¨¿âç·¬ §7¿ìÒÈ'²²«¿ç…¨á$PSRPSRPSR J0023+0923?ÒGoqã}*?Ì°¸NSX?æÜHGAk?Ì°¸NSX?Ñ&5™¹ü¤?Ѻ6?çlå3#®?Ѻ6?Û;¦óöÃ?½LžÓ¤*Ü?âqb,†ž?½LžÓ¤*Û?§·ä3žÅþ?¡Dšéžê?¼Æ ?¡Dšéžê3FGL J0023.5+4454@]oâއ	tÀ1¯X?\6bÀ9 Q¯<ÜÀ;¼fÉbµ¿õ°¸´çÓ¹@ú@'7|n@ŒF JÎ/¿çôª}±J¿å´³5ˆ¿è¿`ÉLc¿å¿½Ù{4AGNfsrqB3 0020+446?ïüPéqÈ>?;VkÏ/®¥?=x´q¾â?;VkÏ/®¢?ïÔ`äì)?õö€ˆÏa?uύ‰øk;?õö€ˆÏ`?ïÄæø?zqÄjõº?}Œüwƒþ§?zqÄjõ®?ïýÿ¡Ï?4ˆÈ'd.?3÷ñŠ"?4ˆÈ'dL3FGL J0023.9-7203@s©_ªŠƒÀFs¡€èTÀ8^½ÇvK·À;f-ù7Žã@¶@)æ®J@ø	24?ö"»J}¿µtDJ‡¸œ¿ÛÍ:°ÕöA¿æš*ž9;‹¿î#J]'OTHERglc47 Tuc?=û‡Ì²>F?7¢kÍÏè?ïü@i¸?7¢kÍÏè?€‹ÃÚÿ?ˆÎ¢€iY?ï½Ð󯘔?ˆÎ¢€iY?~¡¤siJ%?t}ͧ‰j?ï¼·-m?t}ͧ‰n?9¬†_æ¼F?2ÏÃHр'?ïüÊo4)?2ÏÃHр'3FGL J0024.4+0350@[M–ÃüÀM,Úÿ•võÀ:Þ
ò}À;¾Êe€?ðAUÈ3‹@DpýC77@9ÎÀ—à1¿àëÝ3L]§¿æ¼,ÆÝt¿ç¼æç;t1¿åÀ|µ2AGNfsrqGB6 J0024+0349?ïú‡´=)9?L‹h¬oò¤?Eá/[&?L‹h¬oò´?ïßƸŽD?{¹b1à¶ù?p£¸Ýý?{¹b1à¶û?îuãfõ·? !§Q+?¯8¡É¤Œ? !§Q+?ëüÔ×C'?®Fà˜7}?À¯ˆ¢ñ¼?®Fà˜7}3FGL J0025.7+6404@^@¿ã°?õgq¡-ÒÀ9Ë/þËLšÀ;5í£ùo¿À¤®'À•@Œ-ëÉ@±§¶Cž?ëÿ&ò³¿çú
½'×á¿æ;×F£R¿Åoúä¸%÷OTHERsnrTycho?ï^ו
}o?œÚïEÑ?"%
^°R?œÚïEÑ?ê?Ayw`?Ðùu‹gó?Çú"ã?Ðùu‹gó?íR.ÿ=÷?¦ˆx¬Ùs?µnˆGð?¦ˆx¬Ùr?ïv—­Ïm?Œ&Ú}ŸÁ?'-
Fò‰?Œ&Ú}ŸÁ3FGL J0026.7-4603@s½¿ "`ÀQœˆô'À:'–Æ€'qÀ<é¾u5¿ð¹1ø¶Õ@)v'hO @šK`%¯'¿â·4¶&Sb¿é'JO¯j¼¿Þú†¡øÁP¿è.4v)R	AGNbll1RXS J002636.3-460101?ïÿ¼º¬
¢?Ø¿œ.À/?ÑTü—¥?Ø¿œ.¾Í?ïòH"g­?gý9áFê`?[nÖå0£o?gý9áFêh?ïª'-¸œ?†{ £
F?…{›t'ÙT?†{ £
D?ïþ;RºàA?(ƒV¤âdh?,JÔQûî?(ƒV¤âdM3FGL J0028.6+7507@^[òà\̊@( Q¿æ4}À9µ´v"±ÓÀ;™Ž"¬Ï¿ìº+­Wçs@
~kjÝ@»M DC&¿æG9H‡>‰¿ãÄ`óhu"¿Ü`†ÜX¿îÈ·ôoöTAGNbcuGB6 J0028+7506?é
¶ÿ|1?Ƥ‰í~ÒÒ?ËÕ'¤>?Ƥ‰í~ÒÒ?·Ž­þ?°óÖ´<j?§¦ô‡ -?°óÖ´<i?é…Ï•·­*?³€ðlw¼?ÉèÁ©!KX?³€ðlw¼?ï6Ê»?3Ógê?Ú2MQT?3Ógì3FGL J0028.8+1951@\ë°À&ÌÀEYÝà‡kÀ9üaCöÈÀ;Ë«Ä>ˆÒ?åÉoïxð@šÀ`-@x+ßVè¿æ‹ƒˆ±¿à›º%'p¿î°-ʓŒ?¢MLu4ƗAGNbcuTXS 0025+197?í½ÙL3è6?·Ö+
Õh?²5ž`¾O?·Ö+
Õh?ﲏ1O'X?žC¾êìÝ£?ƒ\3¬j‡?žC¾êìÝ¥?ëÂ–;?«Vß=Êde?À÷Ïî§?«Vß=Êdd?ë²´mÜy?¼eÇwg?ù5.HŽ?¼eÇwg3FGL J0029.1-7045@sKÀ]RÁÀG!?©c;À9Žslf×À;ÂDw(UŠ¿ß:]¦Ã@>-_‰¨`@F±_ˆü"¿èm:$¶e$¿áBf=1ö¿à!Ô³mx¿çbN°«ó¨AGNbllPKS 0026-710?ïüìǜ³í?<¹¨Pli?8™Ã`—-?<¹¨Pl…?ïïXUQ…_?i¬iúÎE?`§ª®z¡z?i¬iúÎE?ï'a›ÏG'?‰Ü°ë6q
?‹§™.|?‰Ü°ë6q?ïñûˤ?U¿ËŸŠ^l?\iØ·úu?U¿ËŸŠ^e3FGL J0030.2-1646@X!T€uÀS¢î «†À:ÆÌ؋GÀ;Ôač?Òd
VæÓ@§rëZ§?úZê:GÏ¿ïœ Rc'º?ïÿ™¤ðÿv¿×mÓôv¿Úbêc",¦AGNbcu1RXS J003019.6-164723?ïÿy_ r?eÛõª;í?Ô{ñÈs?eÛõª<m?ïó‹âiÿs?eû±µ?Xè;,8?eû±µ‡?ï°¤÷"r?ˆ¢8EÒs?ƒÖù'ãŽ?ˆ¢8EÒo?ï֐ å›W?rĜñÓt…?t·ï2Tv?rĜñÓt"3FGL J0030.3-4223@sÔÖàL'ÀRˆð€0<À8¥§
›duÀ;¼^¸; ?ÚJ"Õߒo@‰«Ó
@¤ë€—.¿åÚÎÙ¨Ž¿æÒhõk¿é•";
ºf¿çí)]5TAGNfsrqPKS 0027-426?ïÿOlS¬K?ƒ,`¨V?uŠv'¹?ƒ,`¨?ïð"g¯0?jä&^ó#-?^×0Þ¡ŸÈ?jä&^ó#3?ïx¥kc`–?ŠD=]™e?ëR""í&?ŠD=]™d?ïÇ!uŒÿÃ?tøZ´¹T?|oE9€?tøZ´¹R3FGL J0030.4+0451@\Ie¶™…ÀL͵_ȽtÀ7††*QbÀ;8k)«@­ï`J˜€@:֑ó?ÿ,-Z+¿Á7#§=àпÞ°NxR¿çîßNã¿î&Çy­¦PSRPSRPSR J0030+0451?Vßã³öëN?OeßH?ïô&Š?OeßH?Šò;Ø<`?ªއ«"^?ï•È7Ÿ?ªއ«"`?¦
Âq±"r?¤~kKêô?îŸ#ØäæÈ?¤~kKêö?&
–U=¦?(}¿:˜?ïþŸ&š®
?(}¿:™3FGL J0030.7-0209@[¶ýŸÓo~ÀP"Ñ¿æ4}À95eWr­À;­7Ÿ©~?òJß³õ:@qa²øe@V_]2¶¿âo58WE¿åÍKaA'V¿æI×é2¿ïÿÒXÛlAGNbcuPKS B0027-024?ïüÑÈÜå?AÜLMQ?9q¿ѽ?AÜLML?ïòÀö'€?d'Dæ8«^?Z~øûº?d'Dæ8«_?î"ð÷÷™?š×E‡Ç½?§°ð€†n‹?š×E‡Ç½?ïêWÆÈ:Õ?_II 7z?e¨97Å+
?_II 7ˆ3FGL J0031.3+0724@\ŒÿyÈCÀKŽÃ€ðÒÀ: &yÀ;Øöfú
?­òw7aC¦@ù䥆ŒÍ?ý.µÀ@ÍP¿îǨ )z?ëêDE:'ï¿èS´t³¨†?È®?-'_iAGNbcuNVSS J003119+072456?ïò':,Ž?^yÁƪM?Zۋ¦ãü?^yÁƪQ?ïî4(Ä>-?sGtùoK'?aË×;ÁÒ­?sGtùoK*?îÞBçD¢?"Cm]€?¢ыµßÐ?"Cm]€?ïªú"|š?‡Æ¹v8"?…A[ ùYˆ?‡Æ¹v8"3FGL J0032.3-2852@"Œ¼ÀO(ÀU\>ÏuÀ:®1ËT&ÉÀ<âP3ÀÌUàÝ%
@
²gEß]@"! 
Ñû¿Ö{ãaÈ¿æ
8$1Ë¿á¤û|§_¿Ù'ÈÇQLAGNbllPMN J0032-2849?ïûQãUQ?K"Ȓ@¢8?B¸s²ª¹Ú?K"Ȓ@¢9?ïõ—"Hòs?dŽËØuyA?TÐÙnH?dŽËØuyD?î‡T èc"?Ÿk¨ÏæÚl?§Š½ñyÍÕ?Ÿk¨ÏæÚl?ïÿÿËCÈá>™¬TÇÐ=>z^'!>™¬TÈL53FGL J0033.6-1921@W'¿ö$µÀTNW_ÍÅñÀ84©Tø€À:¯8hýœ?æócm_Á@¬¡fítã?ûo yÒ¿Þ¢þIh÷¿ÔÖhW¿Óëm"ΠڿÖù`ïYÂAGNbllKUV 00311-1938?ïú?†ÿN¡?IÀï9u?GäÅ}Ç?IÀï9q?ïíýæ‡	!?kvÌ>kÅ?bxöݾ?kvÌ>k¿?îíùÓ
0?™ú'³nø™?¡ bÏß]?™ú'³nø›?ïî"+¨ ?—¼^¤ÁFä?ŸB;ºŠü?—¼^¤ÁFä3FGL J0034.3-0534@[ß.ßç[ÄÀQº¿ïn¸À8½bð À;›ìVuX?þÍæ°M»@æ`pX,½@%G—ÙW'휿ٿáÕ`•Ó!·¿æA†û‡Jb¿î¨ö4­ºPSRPSRPSR J0034-0534?_Éâ!\½?\FÞ Ã?ïð~›ïR?\FÞ Ã?¸,±^/¢®?Ê蟯	
4?ìúiÔ:«?Ê蟯	
4?ô_÷y?¯Ò—?çU"?ëè¡?¯Ò—?çU#?­"=¡,?x˜ÕPK©?ï¹I³ë	{?x˜ÕPK©3FGL J0035.2+1513@]IP?³t6ÀG»ÒàD²À9OíhMÇÀ;P"Ý?à|[jVWr@¸e{.õa?üç€bæÕ¿ãÓ5»4P¿Ä¯Wíó¯¿ÚCRóà¿ÖEˆ–£+OAGNbllRX J0035.2+1515?ïí(×"'?^ì$žÉˆ9?b×(íÝ}_?^ì$žÉˆ1?ïèNÎ?pÓ´£»*Ù?gëû±1çX?pÓ´£»*Ú?ï6š¢±%¨?'½zÌ_!?™,«©ÛJÈ?'½zÌ_ ?ï
ÕWnö?‰U¿h+?ž¥U!/?‰U¿h,3FGL J0035.9+5949@^?ßÖkÀÙß`£-íÀ83J‰'
ÚÀ:õWÁ‡õ,¿ÌçSÐ{qÕ@÷Õ±Lé"?þ]I^î¢à¿Ó}•?uil¿äÔîuOH¤¿Õò™ûiBd¿×á&$AGNbll1ES 0033+595?ïù‡*
+Æ?YDRñᑔ?IãW×Pâ–?YDRñᑟ?îóòŠr Ð?³v'gSÏ_? À×XÝò÷?³v'gSÏ_?ïqKR0«?½$—Gß?'Ýö•¹êÒ?½$—GÞÿ?ïëYˆ?_¦F"C4?d¦=wïá*?_¦F"C4"3FGL J0037.9+1239@]r7`¿]yÀI
Ô¿àU@À9PäEVÀ;ŠG?¿ÕKÐõ%†@Èé¬+—ˆ@6<6[²¿â	ÚIb¿å¶ì"çʙ¿ÝÂÈïiý¿ã&ã
?¸ÁAGNbllNVSS J003750+123818?ïÿ¸ïpýU>ûŌ_æô3?Ä#ÀªØû>ûŌ_æô?ïð¼]C"‡?d=âJ…Y?^‡ExÖði?d=âJ…b?ïæ'n®§?tÌ÷ëJ'?inâ'QV©?tÌ÷ëJ…?ïðM'YÄ?T^G!TØJ?_dÝMèx"?T^G!TØC3FGL J0038.0-2501@PÂê /JpÀU•IÿþRÀ9ÀF¯ç¹¸À;á"Év7?ãLL@µ>@«õ–?G@'ã@V²>¿åkñ&!U¿å|CåÝê׿ç¤NyhT¿ìÁ‡§Ý2AGNfsrqPKS 0035-252?ïöbÌýHƒ?[ÝD÷ܑ?S:fnúš?[ÝD÷܍?ïêÅøTãC?ph›øŸ?e:«¼$?ph›øž?ïyW"…§?Œ"ã²®;¤?Õ
ŸoK?Œ"ã²®;£?ïJñƒÄá?†o
\¿n?–¡Ï‡cÎ0?†o
\¿n3FGL J0038.0+0012@\ì  ô×®ÀO<¾Ÿã_¶À:[¯ˆïÀ;Õ
»ªeš¿×:]ã¤Ä@'QS"·@@›àEÐo¿Ör:ˆD»$¿æì•^ÃÒ¿Õ"˜Ue§¿åXNRÉP–AGNbllNVSS J003808+001336?ïú%‡û°<?L"3&´Ó—?Già?ö?L"3&´Óž?ïÙ¹–jší?'}>®i¥?s#4ʲ‰Ë?'}>®i¥?ïCjá¢È?Þ"«š$~?—'£ß‹§?Þ"«š$y?ï€î•$Þ4?…5»½Â?ÄZ¶Èr·?…5»½Â3FGL J0039.0-2218@VúQ?ùSÀUp¿ñ7À:ÊËi~KÀ;çåPQQ+?ï¡¿#R%Î@Ë+1¥?ûr"^úŒN?îÚ²ämà¿ág5离¿Ë3^ÿ6Mç¿àÆ<¥ÖF|AGNbcuPMN J0039-2220?ïê}·CÝ^?k®¬ c?e'H¼"¢;?k®¬ `?ïÛ`Ì,Ç?¬Ú3¢?rO¿éœv?¬Ú3¢?í·lÁú?¡»Æ
Œ'?²D™÷'`2?¡»Æ
Œ(?ì¹[¿±t?­I€ ZôA?º5'ât[?­I€ ZôA3FGL J0039.1-0939@\:'@·€4ÀRŠ4fÀ:E$oKvÀ;ß¹Z)AB?í"Ìû=@´¶|ï@ÀsÀ—	q¿ÚR)³W°Á¿êº"vØà"¿í›RÙw¿ïý_"î—«AGNfsrqTXS 0036-099?ï¯åö>úŒ?æ1Pg?"'pA]?æ1Ph?ìˆ]4–?Å
.Ô÷Ú´?¿;½ž[Q?Å
.Ô÷Ú´?ëoH°(¶?­W¼ äє?ÂBßå?](?­W¼ äє?ÙCŒh	
?Á'yÚù^?ã^9ôËûy?Á'yÚù]3FGL J0039.1+4330@^%~0‡‡À3PlÀ»"À:Mq
"À;àÎs•ùÒ?㽝lb@Šz¥7²t?ÿgîÿQ¯J¿éD ±³8¿Á'cÿj¿áÔ?®#ȿݘҔŒê_AGNbcuNVSS J003907+433015?ïÖ~Õ<Ș?wº{{ðd%?tÀ•a›³ì?wº{{ðd'?í«pÒî˜?¾Ÿuynã?²§¤yh‹C?¾Ÿuynã?ï ¦ÜgÿJ?'¿™ÙÔµ×?›ë$sâ?'¿™ÙÔµÙ?ê¶TPƒŽ?°4r'eû¥?Çí&®½ñÈ?°4r'eû¥3FGL J0040.3+4049@^*§"X¼À6J_Ÿ¢ÈÀ:³t«£‡YÀ;³6nQs?ÔuüÎ-†@HG§‰qX?òºÀۧܿç@ÈôfL¿èXBd‡Æ¿Ùîh§Íþ•?Ôð3ásAGNbcuB3 0037+405?ïû²[*?I©.Q©$¹?A7²"‡WË?I©.Q©$?ïÛCæ2)™?}	ÿòÒî¡?r^æë3?}	ÿòÒîŸ?îKöm®%U?£vã(óôD?«@™%ªµ?£vã(óôF?ïÐRÎUã?ypø3w¼Ø?wÖô˜Õj?ypø3w¼Ö3FGL J0040.5-2339@UÊá`ÈWÀUoÌþ£	À:ߍ'ûÀ<ϗ'h%?Ô½
˜Æq$@,҃Åò¾?ÿ#¹€iÇÅ?ïŒp3:a¿äX­šúº¿ä77	¯¨¿¦"ãæ*',AGNbcuPMN J0040-2340?ïþr¼0d?,à]]d.œ?(Ô<ù¾Ô³?,à]]d.Ë?ïõëfY³9?aõ×ޙtx?T)3L™Ê?aõ×ޙty?ï0•^kv(?'=šÙV-g?™íT2';?'=šÙV-g?ïížP~mZ?aX,,‰õm?ba¯'¦š?aX,,‰õl3FGL J0041.9+3639@^4´A»Œ3À:+ä€G¸üÀ:»•EwÀ;÷ÇúÕô"ÀñçßÃ@bg¦'`B?ÿœ»úl?ïþÁVw¿î7à†4¿Å#»L'ö¦?¤»ùë¾ÕhAGNbllRX J0042.0+3641?ïÿµ>QB†?	jÉ{œR?°k¯^ÃT?	jÉ{œÊ?ïëxY¼":?r8óf*?d‡¦CkƓ?r8óf*?ï«O­t4
?€Q¡ó*©=?…,¢òýç?€Q¡ó*©C?ïÿú"]_ý>Û²ž6Û>ÇvŠ€ÿô>Û²ž6Ø3FGL J0042.0+2318@^	F^‰"SÀCÂߥ¥À:‹ ²'À;Ð:‰hÊ?ØÄ·omv%@¥¥À‰d@Õݟ­ÚÄ¿âxj
K(Y¿ç<4–,8¿àn–
ÃÓ¿ïÿÄ^œÌAGNfsrqPKS 0039+230?ïþ)…÷ÁÃ?5d–êG?-g ƒãá]?5d–ê/?ïtL—_?"î¢aåâ¸?'~~ömü?"î¢aåâ·?î¥l+·ºd?›h¨¾d÷?¥©=D"Y±?›h¨¾dõ?í{ùÂÍ´d?¡BV&"¢O?´ 1é'\Ú?¡BV&"¢O3FGL J0042.5+4117@^He¶™…À5‹x_.QÀ9ÛÌ`–BÍÀ;Ç6oþ•?ãˆ=ZmM¥@
kzÜÀ
@¥ŸŒLտṙaܔ¿âÛ
½Wäÿí7ž­)Ä¿âæa(9.OTHERgalM31?é‡R*|œ?ÈÅàøÐ?Éâ·WÆ
'?ÈÅàøÐ?èÂ)8E]é?Ñ ã²Bï?Ì÷[êˆ^?Ñ ã²Bï?롔®…/?±
öåÏò?Áy¯ÍEëD?±
öåÏò?àëZ®¡?ÂOM"œ´'?Þ)J£àľ?ÂOM"œ´'3FGL J0043.5-0444@]rö@c^ÀPâŸÞW9À:‰¤f|5ÜÀ;Èà¨KäÀ
ÉlüX@
'¹Özök?ûÀÝ "šY¿ì5aËÞ!¿Òƒw³¼½¿Ð´
¤¿x¸¿Æ±
3oC/AGNbcu1RXS J004333.7-044257?ïÿD
د¾??ÀÔ-TW?~Dê=³??ÀÔ-T4?ïö‹¡áæ¹?a/çoá7š?Rè¼<2;?a/çoá7"?ïÉ3êé!?w†IȄ™E?{f
‹qï¶?w†IȄ™J?ïÿÿé)ǖ>' g(5½>fÖ8i½b'>' g(´¹3FGL J0043.7-1117@]žYò»ÀRƒ¢ÿßHÐÀ:O".bêÀ;r²¥Z?ç÷ lÿT+@
Aï8²?ùæÀ
¿ïþÏA­Z¨?ïú˜G£Ç¿Ò±á3·¥¿×‰ùÉ/3tAGNbcu1RXS J004349.3-111612?ïû€íH?@…a'ZÝ°?AüJÆÞî?@…a'ZÝÁ?îîBlû?¶ÂÁ'Ö­p?¡ûÞy0N?¶ÂÁ'Ö­p?ïA¡´N°?Œ.-ê>€9?—ËÉ}–)É?Œ.-ê>€7?ç\ ¯¥=X?Á¿è=©DÉ?ÑG¾ µ…O?Á¿è=©DÊ3FGL J0043.8+3425@^J:>À/0À<j'_8t¼À8¾Ž'b™À;Xó"
3¿íÓ>Bä_@žŽ5	L@[ŠI{õ¿Û¬š%8Q^¿ãʽ ßÞø¿ÚxÈՂ¿ã%NŽáã=AGNfsrqGB6 J0043+3426?ïÿ½æ´Û?r‡Évvë?˜†RÈî×?r‡Évw[?ïëEÀØÉ?oÆÒÚ`³?dºþ?'6Ã?oÆÒÚ`¯?ïàoÉ1'Ä?rüÊâä¨j?o6Îm;ç?rüÊâä¨h?ïÿ.µu]? h²¤—>?)Q^tƒØ? h²¤—è3FGL J0045.2-3704@s`—ÿ›V2ÀSý£¿ø¨ôÀ9x/Äé©|À;êöÃ@\¿ää†Ê+@¡aÈ
þ@Wºßd¿åþóX¿ç'¨²¢eV¿å!¢qPòƒ¿ëGóëZè•AGNbcuPKS 0042-373?ïþ\~2˜.?1&à1&?*8Ö}÷?1&à1&?ïöBkJs?_þ#
%‹?S{)kýÆ?_þ#
%‹ˆ?ïÉ÷Õô÷_?y™Ž¿	Vg?{"P§?y™Ž¿	Vi?ïÿJw^Fì?$y>Ukg?±7"¢??$y>Ul 3FGL J0045.3+2126@^CÀh ÓÀD³° F\À8Ú0òçÉÀ;Dþ`Ï6?á!€:ÍÜA@WÛ÷âû?þbw¾þX
¿â'T6@·^¿áOC¢Ê£Z¿Òøx‹›ÃÚ¿ácuxۑ"AGNbllGB6 J0045+2127?ïû;(ŠÒ?@{ŒíiM{?C]Ô·Íj?@{ŒíiMo?ïßìX"=?tH¨;͛Û?p	Ó½·á×?tH¨;͛Ý?ïl·YâS?Æ4ž²?'iߣµ·?Æ4ž²?îàÍ©F×v?d›*?¡ó%k'ˆ£?d›+3FGL J0045.7+1217@^/l?Ä;.ÀIG™¦5À9AvK¶·¸À;n T3]û?ÀŸ.—@ëáwÔ¢Ú?ÿ[@š$¿¹W)˜»ßP¿Þwa¢ÿ–E¿à%Ùºµ·Ì¿áͳiEá-AGNbllGB6 J0045+1217?ïòxî¤?ZµµÍB½?Zá#'+?ZµµÍBÎ?ï獦#Ò:?pw-˜õ‰?hrYÜ-Æy?pw-˜õ‰?ïDÜ8.·?'PÜ÷F?—dxú)w?'PÜ÷H?ïwx%û?€À#æª?'pû_@¥?€À#æ¨3FGL J0046.7-8419@rñŒ¨À@gM@$³>À9Âw»ù?òÀ;¤gHäu`¿ÛÖ'/€‡@'ML @¡€mΐ¿æ"œã·0?¿æŽ8'm«¿ë!ghïؖ¿ïÿŒDÇZGAGNfsrqPKS 0044-84?ïþB—Ž¿?+íé¸c³b?+և$,?+íé¸c³í?ïÖWÁ,Ê?ˆHØ&ìÔ ?~4Ôi›;?ˆHØ&ìԞ?ï"ÆÄÄó?ˆóÛ³ÇØ?ŽÎ|ÎÂü?ˆóÛ³ÇÖ?ïæÕ«2A?'Çdu²Ëu?Œ†J•3oý?'Çdu²Ët3FGL J0047.0+5658@^•[á¨&$À"›!
À8¹R¼ev|À;\ êƲ×?×
Õ*ŒF@=ijý¤Ü@ËC =͖¿åXûRWvñ¿â4Ä¿àR+•:m¿èvK-GXQAGNbllGB6 J0047+5657?ïÃþPïɘ?"™<n8×?~׈4	?"™<n8×?ìüCkº ?Âà¯q›s?¿xä¢+?Âà¯q›s?î–PJp_-?îzÏ#?¦šûXú
0?îzÏ#?î
ÃÀ™¼?Ûìc~ž?¯SÃöd>
?Ûìc~ž3FGL J0047.5-2516@X`ñ7ÀUüæ?Ïù¨À9yEi–œÀ;¶T¶"¥?À7Šïuq@54wž@ZVߊ¿Œ¿âd+Xs^œ¿åFÝA¿Þëqø´1¿æ+
:¥"OTHERsbgNGC 253?ïþ:Ï,L?2
_pÛ?,_£
;;Å?2
_pò?ïßï$Ý4P?~)`ÕPÌì?pm'eØv?~)`ÕPÌì?ïu(SñêÁ?n'"S+?'ZõÂ§é?n'"S)?ïK#MO£?ˆtíÝ#f2?–›–V°?ˆtíÝ#f33FGL J0047.9+5447@^›û'ÃÀ $y?ÜäÈÀ:<‹ÂAÀ;ªU‰ŸP"¿Ó"m|҅ì@.‹@š?õVtªL?îé£%o·Y¿ç²õ «†¬¿â?ñÙ
s?á0êíZr#AGNbcu1RXS J004754.5+544758?ïûÁ† •?PHû\£?@øõç}¬S?PHû\¶?ïaÅc'?¥ƒ–1"Ä?"Ç]"Œ[?¥ƒ–1"Ä?îã=<g&á?–?Gå)—?¡Ì,9'ä?–?Gå)—?ïõœîöÚ?^·ÀÊɕ´?TÆ"ÈL›?^·ÀÊɕ 3FGL J0048.0+3950@^Ž&áY.À7$_ZÙjÀ9ݏRîº]À;¥e5
ÿ¿øbf	aÀ@×)_õ³÷?þna«¿Þús&pà›¿àÇLÏLÀ¿àc¯1±Rô¿Ä30×ÁÐùAGNbllB3 0045+395?ïýۅŸ?4h"ÞEãv?4#Ó'5?4h"ÞEãf?ïèºåی3?u
Фh'—?gE$š?u
Фh'—?E-«¨?†—ß;äc3?‹Ò®´•®?†—ß;äc2?ïÿÞºÓÑ>ô†Öã>ð¢–vÉÀ>ô†Ô¼3FGL J0048.0+2236@^z)à¤&ÀD!Ðß´0À9,ƒöš%±À;™!|QŠ6?îá¾y!ÿÚ@îþj(½¹@ª  žŠ¿Ût'冓>¿æ¥ãµ$B2¿ãíw3µ‡¿ë/EcškAGNfsrqNVSS J004802+223525?ï÷™}|Iˆ?QüÿU_ax?PÍlîU?QüÿU_a|?ïïèŽÆûu?h½
{Œ?`q9‹
?h½
{Œ	?í´Ð÷˺"?¢¹'°Ÿ!¿?²YxA¢+R?¢¹'°Ÿ!À?ïåMñɸà?`$ÓÓi@?j²6G­?`$ÓÓiB3FGL J0049.4-5401@rùm`ûHÀO6@-íyÀ:}2Ȫ(À<Çhß½j¿ÿGDAùI­@ry-hmþ@%µ\Í¿æLÝÏ\&пäcieŽ¿ßúÍì\Š¿Ö ='tËÉAGNbcuPMN J0049-5402?ïþ¨°ñ1‡?,q®M…~R?%tðìç§Ã?,q®M…~n?ïõDlH‹?dl•Þxø?Uw'néÊÒ?dl•Þy?ïµ¹Öyó?',	5(?''˜ŠaƒM?',	5)?ïÿÚEIç >õ²'Õμû>òÝ[/÷.>õ²'ÕÎÀ,3FGL J0049.4-4149@s[6†¥ÀRÓ@ÃÀ:–²gƹÀ<"ę¿Û;óv.Û`@­"óoMì@<zßð&¿æðÊ㓍¼¿êöÇvõֿʪ 1'%¿È9[ã¢ô"AGNbcu1RXS J004939.9-415133?ïÿ|Êc"Q?ó—iœ{?f³•ÞÍ?ó—i2?ïô%ªrx?dˆéÞ·F?W´«ó
¾?dˆéÞ·F?ï'H|bå?ˆà¨PJŸþ?‹­àç[ÆÙ?ˆà¨PJŸþ?ïõÎÓWå•?Pqùq2?TbYP4×ù?Pqùq23FGL J0049.7+0237@^…п "`ÀNJÀ²¤À9h"t¼À;°â`²È?'ãY,@è(©c@óËßgD¿ã,ï!¿äºjþÚ¿Ý0r‡B:¿è<IiÖ]oAGNbllPKS 0047+023?ïÿ'¨iÖ?
í-Q?UåŠ{H?
í-Rœ?ïîâýuSõ?k%jŸ'±?aŠ¬ð?k%jŸ'·?ïÂï̛†.?jZm…?~ˆ²<éY?jZm"?ïà"–'#ù?bŽ‰pXÁò?oÝiØÜÒ?bŽ‰pXÁÿ3FGL J0049.8-5737@rõœýç!ÀMÀR@>´qÀ9ҝë7òÀ;ØÌð;8¿½Q‡Ðw@‡ùZ"z@²'€Ê÷¿èà{ô-å¿åòˆá±O¿åîôŒÚD¿Ò®D$ТAGNfsrqPKS 0047-579?ïúÊ%R¥ƒ?HGFQé×?D×jµiù?HGFQé×2?ïòF/(ј?g¾k;Ìþ?[s¡®\ÐM?g¾k;Í?ï"ÂnàX?ƒ&ÇÊA?ŠÏdGø*K?ƒ&ÇÊ:?ïÔ!Lpä÷?ló°+ûÝ!?uïYǍƒé?ló°+ûÝ 3FGL J0050.0-4458@rû¯_Ô{îÀR	â H¤À:NÈ>Ȓ«À<Üq…~Z¿ãP€èa—Ž@è«,¾úÒ@9Ÿ…@ò¿ç³Zh‰à¿ààêZɜŽ¿ä*NãgîÒ¿ïÿ—w«];AGNbcuPMN J0049-4457?ïìfágw†?qy²^½,?c™˜ˆz]?qy²^½,?ïïA*%Q?m*è.M¸Ž?`¾ÕæÚ¯?m*è.M¸Ž?ÿߺ"?Ÿ^Df?§Öð]Ã?Ÿ^Df?ïìŠå¸Ò?^¼¶´12?cuG-àœ?^¼¶´1=3FGL J0050.4-0449@^"¤as¸_ÀPìû_ò®ßÀ9ž±ý=­àÀ;§Ôî~:¿Ön>ڎà@'
ǾÅù@™\ÀJ]q¿á—:f®4Ü¿æ"Q¦ùT¿ä@Î>p´¿í"Ó_Å|AGNfsrqPKS 0047-051?ïôw"¤e©?XÞ>4…×?Wö·4¯T?XÞ>4…Í?ïáäK<?zGå*J?n´ûÃîˆ?zGå*G?îŠýoø?œm瀥–Ø?§P.©~â?œm瀥–Û?ï©kQÜêá?|3)h}Ùñ?…¥+ˆÅGñ?|3)h}Ùñ3FGL J0050.6-0929@^•-û¹ÀRÄ`Á
À7ï;M;À;
;…è?ÌÚ#ޒ®)@ø‡©'ö@¾ž²gÇ¿Ýè%Õ#¿âËÿóγ¿áíT<ÿK¿ádiÛ±ÖAGNBLLPKS 0048-09?ïÿ{Sn?!½Qúq
?•'>}ùó?!½QúqV?ïõ×õ°6Ž?aAy¿C!ê?TPŸ'äÿ?aAy¿C!í?ï¯Îa?ƒ@'ìú1i?"}úç¼V?ƒ@'ìú1j?ïÿL0n?ðmhÎ?ÿÖyòjÍ?ðmhÕ3FGL J0051.0-0649@^ª`4óþÀQlÆøÀ9'Þ³íÀ;€X‹Ž>?öÛ)üþ˜Í@]‰~noõ?þôwÉe9@¿ÛÐ\ùпäñÕøO¿åwåiÑ«¿ìh­ø AGNfsrqPKS 0048-071?ï«äP¥4?ƒÓx¥ßhÿ?…8†ëÖ²ë?ƒÓx¥ßhÿ?ï+¯<?i•†Ê?`nVÔPÃ.?i•†Å?é¾"}–N?°Œ#»mR?Év¦Å?°Œ#»mRœ?ï'-YÂ?/v ]Íâ?‹t©`:q?/v ]Íâ3FGL J0051.2-6241@rïj_"ÊÕÀK8X R…ßÀ8Ô¢ŠÙã6À;ÝS¨?ãiËÙìÙ@SBïòÌ?úœF__áè¿å.w†Á¿Ó3h7Kñ›¿Ì{fLTU¿Ó)ÈÐ,ÂpAGNbcu1RXS J005117.7-624154?ïï}!¨†ÿ?]1R<´L?`'ÞWy?]1R<´N?ïíSõÄJ?hёPñß?b¬ð
;µü?hёPñÛ?ïÃpýä?"Ìfîk?ŸÇ'ÿ Cs?"Ìfîf?ï&^á¸Jê?í0pY‡?›4#Èö¢Ï?í0pY‡3FGL J0054.8-2455@aÐØ`fÀUêeà.©aÀ9G±CÝ¥À;Ph¯ìÂ6?ÛgÓ`¸@ÕÄÉH3?ürå?µL¨?íš®t>Ž¿Ýb=ºd¿Ó<ؘ£Ù¿àtuȯAGNbllFRBA J0054-2455?ïè
:û<ü?gu`KÊ©?gòÅÃÇ?gu`Kʪ?ï讵Áá?sà%ƒOZ?gQJî>¶?sà%ƒOZ?ï>ÇWâ"?Ö;@jöá?˜'U»Æ?Ö;@jöà?ï1ÓBñÉ?
;§_?œYŗ¡ÆÇ?
;§`3FGL J0055.2-1213@_ ©?)
»ÀRÄÿ¿ÓÀÀ:xHG—nFÀ;ö
>¬ãù¿àÓ|¶¬F@ìŸf7A‹@,€0¥¿á †N
!¿çÖ´ñӆ>¿äü—öV^¿ÛºßáÛíAGNbcuTXS 0052-125?ïÿ½"¸?3½±?›ÿy§H?3½±á?ïöOȾ%¸?`òýÀçœ?S`nƒ´&?`òýÀçš?ᄊÏpÞc?€-"uöõ?€RL#Èg'?€-"uöó?ïþ"™um?'ò½º§b?-Öh©/®?'ò½º§b3FGL J0056.3-2116@`½ë¿×ÀU
€!"À9•ÄÿxñƒÀ;vÖ
c0Q?àÙo@`Ö#7½‡?üí~@!Ù? ïÃ
J/¿ÒºJ†-x¿ÛÅð Í§¿Ù×RH'ÖAGNbllPMN J0056-2117?ïøŽOÜ*?S-Øwÿ>?MÆÀñS%?S-Øwÿ8?ïñ­Üý`Š?f8•Öš?\¤F>ìÂ?f8•Ö§?ïq#Iì±¹?Š½/ƒn-£?'Û–ÂiÈØ?Š½/ƒn- ?ïœäuÉÀ?t…!ä–úw?ˆÆú¢³?t…!ä–úw3FGL J0056.3-0935@_½^	ÀRSÍ$áÀ9ÁÕùµcÀ;|Fûg¿³Õ¥½@8@7s'À?ü¤À Áìt?ìÏ96Ç+¿Þ$ÖxQ¿Úç0‹c ¿Â^P»HAGNbllTXS 0053-098?ïþ"xª±.?(	žs©b?&¸uTí-w?(	žs©M?ïõ²N€?c"vw¶ô?T›câÿf?c"vw¶ð?ï°d…<!?€úõm§îX?ƒÿ&Þ°ø3?€úõm§îZ?ïù°Pµ+9?B•Ö3w?I>½+SË?B•Ö3}3FGL J0057.9-0542@_ÖNaŒâÒÀQ!ŽèӔÀ:43#Bû'À;¶Ï†»p"¿ïzI²‡@,
{®÷û@R²à£¿à¼‰ô
(x¿æÒå•Ò¿å_ï˟J¿æ¤´ïz;AGNfsrqPKS 0055-059?ïöjÚ[A?YIçÀñ4I?Sÿ*KI}²?YIçÀñ4G?ïò‹g•?fïï{¢>Ø?Zé0zÕð¨?fïï{¢>Õ?í¿Í±'O˜?§^ün7!‡?²'smƒC?§^ün7!ˆ?ïõJlº£?Q›eøNp¾?Uk&ŠÞºC?Q›eøNpÌ3FGL J0058.0-3233@r	€bïÀU¿ÖDEÀ9C'5ÏÆÀ;€Æ'—¾?ï+I˜¶€ì@¢Ž>F·Ÿ@w~?ËòÝ¿Ü«#ñ2¿ÞšMìût¿ãX^v‹€/¿âm+©û~AGNbllPKS 0055-328?ïóþYç:«?`(
ÆU?XL1Š¨G?`(
ÆU?ï±YSG9ý?"°Ù¸‰³?ƒ©«.1€Ê?"°Ù¸‰²?íë©›å›?£¨H΢/?°¢·Ë Ó!?£¨H΢0?ê×XU?´4šÄí?ÄõÀ£¦žª?´4šÄí3FGL J0058.3+3315@_%þKZÀ=•2¯ÈÀ9ή"i›À;й!õN?ÑÞüûÛO@ç0+kéˆ@B"@Îé¿æTgê䩧¿â.ñ°¿æ[š6nô¿íËLŽ'JAGNfsrqMG3 J005830+3311?ïĆØdh?|fû²®¡?}¼"öÍÌQ?|fû²®¢?ïÚ®!éÜp?yOj@/
?r¨ïÈx?yOj@/?í¢Í‰A5?¥šÀËÃ(	?²é"µöWë?¥šÀËÃ(?ïÉK²ŒT?lŸ-@?{Z&¹Õò&?lŸ-@3FGL J0059.0-7242e@râR€jôkÀF5W¿ÚvÀ7îjCj¹À:ô‹…à_?í]ñg¶È@AT;9½@đ #a¿ÛÆ2x'É¿ä•×m9¿>¿ävôô3C#¿è"äÞ¼csOTHERGALSMC?èð€ãD?ÄÀ;2ún5?Ì=üsâïš?ÄÀ;2ún5?ÒãÛ¢ÔÍ?к\Ž?æŽz.•š?к\Ž?â…o¨Gð?¸Å9(
?Úõ!Ò¯p!?¸Å9(?É!QRóà"?µ½qéOvq?é·««Cø?µ½qéOvr3FGL J0059.1-5701@rÍÆøÀN	T9À9~@¡°À;ÉS¿šµ?î°–7@¨•žÃû@îpnö¿ÞTíPo¿ç•>&þ¿ëH_TÉ¿ïÿåώY[AGNbcuPKS 0056-572?ïìóèDë?hY[·ùÏ?cà»9?hY[·ù×?êC‰=>p?ÇÊ@oÜÎ?ÆñÛó@?ÇÊ@oÜÎ?ìLËY©åw?®e-`?½™¥2°ÔE?®e-`?Ýà	¸´ß?À¨° ››?áú{#¥?À¨° ››3FGL J0059.2-0152@_߂¡/ÀP+á .QÀ:k+D´À;½¦læ³(¿Ô·Qª0"q@ï9}$C?ûÍ[ d¹é¿Øµ{!‰g¿ë´kÏhç?»¹=ìÓ0¿Í²w°}þAGNbll1RXS J005916.3-015030?ïÿ	ã))?!8?à8"?ÚÚÜ·¶?!8?à8Ä?ïôÚN0,˜?adÕ6Qà?VKcŸ¦Óm?adÕ6Qà?ï¢ÏlÀÄz?ƒèívßNÐ?‡L$ÏÎá¶?ƒèívßNÑ?ïý#"¦ÃP?6cSöŽ†	?6ãZÉå{r?6cSöŽ…ü3FGL J0059.6+0003@_ÙØà†8ÀO_Ï¿ÆT
À:J'ÇÅ&À;ϸé?á÷÷ßA'@¢éCÐå5@ß&_3i¿ãÓÕ!&Ž¿æ5h¡Bõ¿çÀµQRzn¿ìŠðð~¿AGNfsrqPKS 0056-00?ïÊ"¾jó?ƒ®c"³¾r?zîñ ʆÍ?ƒ®c"³¾r?ï²ýï\úÇ?á€­;x?ƒ@"(ÁNS?á€­;y?îaŠÐ'ó?œs4ÕJpî?©çRýŽÐ?œs4ÕJpî?ë.2Ws}h?©]ݕ—$¼?ÃG6¢2
`?©]ݕ—$¼3FGL J0100.2+0745@_°4?¢­?ÀK…à
—3À8«sp:$¿À;
{¬HÈÇ?óîCÍ_CÝ@«wènê?ü¾ÌßAC—¿ÂhÍÿ|Í[¿Ó¾Å4ts<¿Øw=N?(¿ÛþNuÀÒAGNbllGB6 J0100+0745?ïþßqges?0Û,=I½?"鉨Ñ?0Û,=IØ?ïì`ó1He?poß¿ö?cŸηšÞ?poß¿÷?îÖöõÅI?š™[ý14?¢žð£«j?š™[ý14?.G³?"ßýÅŒ?¥FmŽè?"ßýÅœ3FGL J0101.0-6422@rÓ[ߏG0ÀJ\ŒSâÖÀ9õ[aO¦À;Ê~ÀÐ?H?þÃ	õ¢.@
~×ÌZ6@FÂ5D/…¿Õ€ÉÈ¥9¥¿Û'hÉþÅ¿çM‹È>H¿î+
Ö
áPSRPSRPSR J0101-6422?bãÙ_Ñ|?]uû°™Ã'?ïí& .ƒ?]uû°™Ã"? Å9Cè?¤IÉ»òy?îó¬kÁþ?¤IÉ»òy?›+öΎû?˜<%póÑ?ï& O‹ˆ?˜<%póÕ?•úhTöàu?µHI4î?ïP,½XHû?µHI4í3FGL J0102.3+4217@_Eð¡¾+IÀ4‰xmžiÀ9SDñ¡˜À;Â"³‰.è?éSGà¿Gÿ@š€Ê?Õ@ˆˆŸÌ8¨¿æÔŸÚrÊ¿èžr!c/®¿ë…܇n¸‰¿ïü-êì>úAGNfsrqGB6 J0102+4214?ïðO}˜0"?hVYvÜ	?_aϞØ.?hVYvÜ?íŒcÿVÐE?»b¾Àƒ7ß?³œàI}Þ?»b¾Àƒ7ß?ïX@>?Œ4ÛÍH?"ýÿ×ø ?Œ4ÛÍI?땇ߕG ?¯^/‰?Á©àªã~?¯^/‰3FGL J0102.8+4840@_7ƒ]íñáÀ,Oö¿ž(À8ÏϚ¦ãÀ;MIðäÚ
?úÝÙìD@­AÂ<@œuhâÿã?‹þrى¿Û®Ó朂¿å‡)yù\¿ê-s>¢8`PSRPSRPSR J0102+4839?à/Ó·Í?©Ž&?qú?ïˆ@±!Á?©Ž&?qù?¸SLJvN?Ãr8…qì¦?ìõ–}–±7?Ãr8…qì¦?Ã82òo	Ì?±h"~±#?ë1óCd=?±h"~±#?°nX}À£?š.¯lQõ?íò="ðGì?š.¯lQõ3FGL J0102.8+5825@_B€®IÀ¨!ßβ*À7‹dBSbÀ:ú3ºA¯Î?ú‡Çßþù@;ºjŸ†@²,±¹Ëé¿ÝƬ_¢…"¿ãÔ"‰Sw¿åЭh>¾é¿æÙ¾«T‹AGNfsrqTXS 0059+581?ïÓ¥ãnqÄ?tµëU1^?v-HÇv?tµëU1Z?ï¬dD?°ž~wmÈ?ŸJs×~+?°ž~wmÈ?íKèÍy?¤e׶?µ£¿a"??¤e׶
?ïÿYD?'IÛ¶Ž"?ÌW"?'IÛ¶Í3FGL J0103.4+5336@_/0¾
í)À"mµ'm,À9š<Z#bÀ;•µav<¿õr`''èu@®µ©D²@Oë L'(¿à…Œ¿âõ¬¸}¿ßµë–³Ø'¿Ô=ڟ%þAGNbll1RXS J010325.9+533721?ïóbGüV%?V(9»™ôi?Y;pS³Æ?V(9»™ôk?ïs\‰BKV?¡ÏÓNÇíÚ?'"n׶•Z?¡ÏÓNÇíÚ?ïX:!é*?¯üÖÄÝ?"ýØ»ÂÚÚ?¯üÖÄÝ?ïþËý™&u?$­òBÔúß?#@&m˜ÈP?$­òBÔúÿ3FGL J0103.7+1323@_âx £
·ÀH¯8à^*À:-m\ú¬ÚÀ;ËVN?ì~fº–Œ@º"kì­?ÿ½'ÓY¿èGr°K¸?––á"–5È¿×Q\`uƒ¿è?iÔÉúAGNbcuNVSS J010345+132346?ïÉà¯æç»?}"e_ƒuØ?{¨Œ"Q?}"e_ƒuØ?ïž\áÉ¢ý?ñG¬Ý©8?ˆhǍ—@ø?ñG¬Ý©8?î»×Ùnƒ?¢ÙÑM
×?®ÄB'iÈ?¢ÙÑM
×?ëyp‹àG?©€«¾Ž;X?Â?ÅÐ~å?©€«¾Ž;X3FGL J0105.1-2415@eZ`˜ÀUréÅ+À9jÑáÃôÀ;Üó…ô¡?뀾iW@@(4'@Ý砍©¡¿åË,AZ¿è'þO{¾<¿èåx.(Ì¿èΆ¢éE÷AGNfsrqPKS 0102-245?ïþ@q­/?.
.±'Õ?.;øå-Ç?.
.±'?ïÞK(?¾,?ƒÐÎ[2a2?pÚkà éb?ƒÐÎ[2a2?ïUµr|)?Ø˜
Xã?•IQ¿zÐ?Ø˜
Xå?íKæC[%S?§íÕà'
~?µ Íå&Õr?§íÕà'
}3FGL J0105.3+3928@_va€M˜9À7R_>SùÀ9î㾀ٯÀ;Þ
,8m/?Ó,×(ñ:ë@¼e$@›|ßy¢®¿æO¶{ý|m¿ç´2°	%K¿Úµ†HÂb¿ì@÷33™AGNbllGB6 J0105+3928?ïùJµÁÒ?OV(y?JÕ(ùȶ	?OV(p?ï²±òª'ˆ?'ˆuWJ²?ƒSƒUvM?'ˆuWJ³?ïH? ³?'ãW¡*%?–ý8é•?'ãW¡*%?ït½Fu)-?…†»«?'hW1Zڀ?…†»¬3FGL J0106.5+4855@_^́'²ÌÀ+¾øßzN{À8®=Ç᫁À;Sà0Vßá@Úi=DY@
֛©"8‡?÷T™"öÊL?èÃQ¿Ù(…ÈßàÙ¿áêe¿ïá¼hÚ·PSRPSRLAT PSR J0106+4855?b9ê  ?g

É¢¬Y?ïíÆrß`?g

É¢¬X?g²"•ž›8?{}éÓdxÎ?ïèMljae?{}éÓdxÎ?ÈeWò³?Š©ýR¼îÃ?ï€Þkæ 7?Š©ýR¼îÏ?g&"OUèÑ?`Cê²Qo?ïèÙk°ª?`Cê²Qo3FGL J0107.0-1208@a.T2TçÀR¤• Õ`À:l,µÿ+À;äkŽÄS'¿¢—z\Få³@åN`¶#=@qŸš´¿æK£ê«Z¿à>'$e™¿ÝVÎ:WŒ¿ê±K}"÷AGNbcuPMN J0107-1211?￵MS1?ƒ—)üÂ%1?€¬«3¹5?ƒ—)üÂ%2?ïµ»b"m?ŽÙ°e¥¯Û?'''[$½C?ŽÙ°e¥¯Û?íGǬ´×?¨ õ)"?µÇÑšYJ?¨ õ)"?î6/Ú?˜"£(8æ?§îo̝R?˜"£(8å3FGL J0108.5-0035@`Ž2ßP]ÀO"!ÀD(NÀ:_-p{"À;ÍaÐÕp	?ç*Î$20Ì@$È´º1@&H «L¿à3×m5¿âÆïD4Ò	¿êÃPċ¿ïÿLˆ¼ AGNfsrqPKS 0105-008?í??26þQ?µˆõ˜!O?¶nH
}?µˆõ˜!O?íòÍY9J?¾ìWßށ?·i•65²?¾ìWßނ?éÃkT"N?±V|J[¿Ä?ÈòR¯ÃvË?±V|J[¿Å?ágõÃÉÆÒ?½}¸Œ?Ý0xlr\?½}¸Œ3FGL J0108.7+0134@`{Ãá`xÀN	@¢CÀ7yÚh–ÂOÀ;Ù}µ7…?øn$Ù(OÕ@kä)µ°ü@Ÿå]½Jy¿â ÞÀŒš¿æ¶­ôøîq¿åe³™ÜÚ¿ê+\üŸBAGNfsrq4C +01.02?ïø@Ð×>€?H:4ÞKuk?Nü¼£5?H:4ÞKu]?ïòȸØsi?e9Žk‹¥Ÿ?ZnŽO/"?e9Žk‹¥¢?ï	|©	™q?•áêG^?žÐjÞÌÑÔ?•áêG^?ïë8‡?hÄËÓA¡?dãìæÇwî?hÄËÓA¢3FGL J0109.1+1816@`çßã*ÀF3=?üoRÀ9ÌjNRsjÀ;¸a†,ÕK¿â@2,…Ú@
§Ü"@k@Q–ߪõâ¿âÇ6cݿׯÛ[A*~¿âðÄQOû¿ÓÔèÍçÝ}AGNbllMG1 J010908+1816?ïýÖ	îÕ?7~Õ«Ò k?1O¿°‰["?7~Õ«Ò Q?ïïÖÈeÊ?h-˜s°«ó?`ï)7š5?h-˜s°«ö?ï]TÆ??ŒW½7›´?"U}‡8µ?ŒW½7›®?ïÜ)ÔÜϊ?n•=ä9œ?që'˜:È?n•=ä9£3FGL J0109.8+6132@_H?Ffí¿óååÀ
̜À7³Ä UàÝÀ;TáÙ¤?ûÊÉĕF@µ|Ï'@'X³ö<2¿ãáÕRàÖ"¿ç?ÄEa*Š¿ëö•¿è¯ürŠi®AGNfsrqTXS 0106+612?ïÛªMÛ:?uÍ肛ãƒ?r*Ùrb?uÍ肛ã"?çk]¸$;ø?Õ%î¨ñæþ?Ñ)D·ˆ?Õ%î¨ñæý?퍔ú#H?¡è8žI?³"X.çíÐ?¡è8žI?ïüæœH>Þ?=»ú Fn?8˾	X?=»ú Fn
3FGL J0109.9-4020@qÿ4?¢­?ÀS¿ä†þÀ:]Y#‡Ä…À;ÇOr.Å¿ÿô
]ᇚ@
~	æ]Â~?û£l`üD4¿îë]£–"ú?ï¾âá-¤J¿æÏÊ|ª9i¿ÉX­*ÅüNAGNbllRBS 0158?ïû%©ù±?BïËæð§*?CiXù>Ø?BïËæð§?ïôo9â-â?dÔ)÷U+Ñ?W!Œ;¤8É?dÔ)÷U+Ù?ï9ZYø˜?´ÃIID?˜Ô´ÀìÿU?´ÃIIC?ïÿš[|[5?)µ™jO?	i é2T°?)µ™i§3FGL J0110.2+6806@_,‰a=1º@;N¿«§
À8´¿%DÀ;´öí1Ç¿ñÒف;)@Æp÷cú?ÿڑÿFq©¿Þª¯ iú¿âq«h#*¿ßíž
¿Öì,39¾=AGNbll4C +67.04?ïáÀ¼ö?dC°¯€!™?n?C÷	q#?dC°¯€!–?ï©hÐ\ß?–HõŽk='?…¥ËèÈ9h?–HõŽk='?îœ\"Ûɬ?™Iê
•ïA?¦:6²Ce;?™Iê
•ïC?ïãä˜0Žã?s]SXÂ?lgÏqS?s]SXÁÿ3FGL J0110.9-1254@a¶êá‹ÀRÄqýÌIÀ:pµÈ¤I À;Ó	¹½&¿ìÒÏbJÅC@ȍ¸dàÕ?þÍÉ¿|,K?Ú#pqpõO¿ÚÁÜÚ$¿ê30ïꑷ?ÊY1y´™AGNbll1RXS J011050.0-125455?ïÈmŽD"?€/ LӁ?{É8ݽõ0?€/ LӁ?ïô_…÷¢:?d†Ø˜€+?W@ô»<?d†Ø˜€+?썥¦ó?ª	]}R?»'ÔÏ[?ª	]}S?ïùÂÕªÍ?Nò,"CóP?H÷è©TÉä?Nò,"CóY3FGL J0111.5+0535@`ƒ'ßüTzÀLvÆÀCQŽÀ:"#bۗkÀ;áž*øÒ¿Ï@h¡DB@»»+9¿"?þ«®>Â2•?츝ü]fÁ¿ÙqÃÇj=¿ËåòFÈ«¿â(4æezAGNbll1RXS J011130.5+053612?ïýՉD`þ?:lÕ$–îŸ?1SµÜøž?:lÕ$–î¤?ïòÒ]E¦B?d6
À©:?Z[Et³w™?d6
À©<?Éj¾?"ŒÙ-'4þ?ŠÑ͹ePÄ?"ŒÙ-'4ø?ïø ˜&?×?EÌe"¸€?M}Ÿg¦®?EÌe"¸{3FGL J0112.1+2245@`$›«–òÀCîŸóOîÀ7FëÝ3L^À:£!
;Ã%?ø>§UCÿ3@Å~öU1?ýøã
Hٿ؜t/ó¿àäJ\Å}οáC€»Û¿ã´¼~å§ÿAGNBLLS2 0109+22?ïû¾ÉÏj0?DP}:‰¯u?AØÂW>U?DP}:‰¯ ?ïî…þŠºŠ?j	øªÉf?azuEv…?j	øªÉl?î'b5Lêo?šWܟZR-?¦éÜ«1Y
?šWܟZR/?ïíÏòÚÁ–?_Ué³¾Oy?b0
%>j"?_Ué³¾O~3FGL J0112.8+3207@`)?)
»À>†§ ÃY‡À7ùpQ¡³DÀ;]*Ãøèµ?ç Ü ›×@räOOt@æšà@œþ¿ã|Tò+¿å{{°iX£¿æŽ;@Œ¦Ü¿å±ÿaýÿAGNfsrq4C +31.03?ïû‹Ôa#1?>µà=j‹l?AЮ{s;$?>µà=j‹p?ïî¦ÏUbU?i?Ú¡7?aY0ª©í?i?Ú¡7?ï•»hH?"0ÝÇã?Ÿ
]h'÷?"0ÝÇá?ïÿÒe›P>ú¨fs=°ý>öÍv²XjÀ>ú¨fs=®.3FGL J0113.0-3554@qJ@WÀTLŸëÃ2À: W À<¾ne8i¿êøü^=@´½uÁÎ@ÈŠ>ˆ¿äGÃ*.C¿äódfº|Ç¿ïv­×û:Z?åeä J…,AGNfsrqPMN J0113-3551?ïÿÏ ‹^N?¦¢ç´Ðý>ø/ºPÙi€?¦¢ç´Ð?ïö>ûŒ7û?`¥Îáż?S'ç
?`¥ÎáŸ?曆äŸá?†™ìÙð\?†]Ø9ð?†™ìÙð_?ïÿêL—BV>ó!í,oMh>å³h½©L¥>ó!í,oN 3FGL J0113.4+4948@_¥>¢ŒÀ)Í*Ž:ÁÀ9I݂&¶MÀ;ŒÚF2y?–ªnxåŒ:@æì·£ÅÂ@dŽÀ!ß¿ã¦oÓ¢~ð¿æeí;›ü9¿ââëYͿ൮#O¡AGNfsrqS4 0110+49?ïé)ð'?têšÜ,÷?fÖäåmã?têšÜ,÷?ïSAa=¨õ?¡I'xO{±?•—ÓØJám?¡I'xO{±?ïöž"·ó?–Ÿh#È ?Ÿ!,;©Œ?–Ÿh#È '?ï"c΍¦?ŠI‹½6•?›¼S†.Kh?ŠI‹½6•3FGL J0114.8+1326@`tÿ´€¦ÀH…>ÏuÀ8õ¾smµæÀ;oU"‡"¿ü¸0ÆFuÛ@wFwÉM@žL?ž¦t¿×dÄ9Lʿ怲u¾æ¿Ýe­›{"l¿ØtiD£YGAGNbllGB6 J0114+1325?ïÿæ	,Šl>ç™tLz>éöÓu"Àä>ç™tGË?ïôÿ""Ê?b?°`_?VþÙºj.?b?°`Z?ïß Äæg¯?t¦v|ª2Å?poŒÌ(2?t¦v|ª2Å?ïÿùÜ$F>ÒÞÆKnq>ȏnçîËz>ÒÞÆKn3FGL J0115.7+0356@`Ѿ ºKÀM0¶ßû}ºÀ9	ÓöeÀ;xÃkúúÞ?³©ûæ"°Å@[Î\ïÅ@ñÌ )–&¿ÙÊ.Ýc¿æ€=Ÿj5¿Û°üýl&ð¿âþ3¼×?AGNbllPMN J0115+0356?ïøþ"3½?QNj¹oþ
?O˜ï1
?QNj¹oþ?ïàýlí?u5\µ¸£?oû"ù?u5\µ¸¡?ïXþڏ?'ÍÈm®°?"à$®Üâ?'ÍÈm®±?ïV $*ù%?…õ€7å—?•;ûz ÛC?…õ€7å—3FGL J0115.8+2519@`;[ߏG0ÀB›dÜY2À9ç
¶<À;aìNrSÚ?á«ÊžŸ=@Ù»$Ù©)?ÿÊW!O!¿åޛâi¿às݅+Îe¿ß>ß)×Ðó¿ÔkêÒÏνAGNbllRX J0115.7+2519?ïüt´ÌxØ?:6ښˆü?<ZYœ9=Ì?:6ښ‰?ïç»4þã?p¡oÝn'r?hDË?p¡oÝn'o?ï£ê³~¡9?…­ƒíÏ?‡S W±È?…­ƒíÓ?ïpñÄyá?€öÍ)¼–x?'áÏÇpÃÏ?€öÍ)¼–y3FGL J0116.0-1134@btÀœ<âÀRZ?ßéàÀ8ê`ão¦À;¬\ê½?êë5·¶©å@®!èÝúr@ÀPÀ6çH¿Þ.ëlcð¿ç´Ak	¿æ¡g"âöZ¿èRàÄjAAGNfsrqPKS 0113-118?ïþà!Í?'ª½Åâe]?.¡ýã.dL?'ª½Åâe$?ïôû§{Ÿ?d'c©ä»,?V±Áۍ?d'c©ä»$?îÇA¾ŒØu?—E×B9¬È?£‹ä2x°?—E×B9¬È?ïþÿ8…!§?K´)¸Rš? w­å‰Y?K´)¸R~3FGL J0116.2-2744@k–PÉSœÀUM`#UÀ:jâÌéRÀ;ñ[dR?¡ZT¤
ûu@
—&`çÌX@.ÿ—ÐA?éÄ×Ä]Σ¿ÞɌráì;¿äƒT¸þL¿Ó¦ýÇãÑCAGNbcu1RXS J011555.6-274428?ïÑ4óÄ-¢?©"Å_¾~_?we†é/	?©"Å_¾~_?ïñâʹº?f–Âã¬É	?\:kÀŒ?f–Âã¬É	?}#—ñ?š)5ÿ˜Ò³?¥È-Ɓ?š)5ÿ˜Ò¶?ïÈEî#™³?sÛLí·q~?{Ýî3&H?sÛLí·q{3FGL J0116.3-6153@rœû`(^ÄÀK~'Éä»À:ѵiÙ¸À;å€~?¡¿©M -Ì@¹"x˜B,?ÿd¿9Ú¿ÝCbB"#¿ådá¸['¿áuÎw¶‰®?"%µy҇AGNbllSUMSS J011619-615343?ïýQL?@,(ïc#?5sŸÓå?@,(ïc'?ïôÈñÉ]5?aQ'ÂÞ®É?VnmE"œ?aQ'ÂÞ®Ê?ïŠByb?‰  ê·[­?oa¼'y?‰  ê·[­?ïóv¦Åç?TÍ΀_¤?Y²t0þt?TÍ΀_«3FGL J0117.8-2113@e:Œ¿+#šÀTdŽà3·À9Is§—‰À;>e§#ÅØ?æj³Æ§ªæ@Ÿæ:@"Áÿê0‹?ÈÞ÷5šÛ¿çpws¡YÏ¿ã¥yéï¿çKÓ µ'AGNfsrqPKS 0115-214?ïý—?–?5Åû±xè·?3G¦OZø?5Åû±xè½?ïëJ ÿÊ÷?tîæhää?dµ_5
­?tîæhäà?î²­@[K?˜z[PÈ@ò?¤Õ+úOT?˜z[PÈ@ò?îÕùé܏W?Ò–L­{?¢ ab7
"?Ò–L­{3FGL J0118.8-2142@e¬Ø'tÀTorßñl¿À8HK"bаÀ;ô3C#k?ûÿaw>Oò@½ßtWj@š*ôw¿â¾¯CAk¿ä֛:…¿äá§fz¢!¿éþœJwÈAGNfsrqPKS 0116-219?ïÄ(?r2?'R§X2†«?}ëàFæôÒ?'R§X2†ª?ïòi ˜»T?c1ì·ÿÔ?[-¾Î‰Xâ?c1ì·ÿÓ?ìρbý"q?§>?œU?¹ƒôèìu?§>?œU?ïà±äb‰?–ÑézÈQ?ãéÃs®Â?–ÑézÈQ3FGL J0118.9-1457@cl O*àÀSt`$-À:Q¹  À;Ȭ¶¬Ï׿º[Ï@'âã@
]7Ÿ©~?ü"Ëÿrfz?ïŠeöÔÞ¿á†áÖÃ-¿ÞœÎ¤µ¤¿²8}4‰¢AGNbll1RXS J011905.4-145906?ïþj
zØ°?1ùC7vHã?)_(Ru?1ùC7vI?ïöÿ€«`!?\ðîÄ +$?Rþ©?À;?\ðîÄ +!?ï'GŽˆËŽ?ƒáü¼
ob?‹n]Íh?ƒáü¼
o`?ïñõbàÓ?Uˆì¶€5?\:?â[?Uˆì¶€E3FGL J0120.4-2700@j²¸`™ËÀTáþ@_ŠÀ7âW5ŒªÀ:ÙP·¨xZ?î¯Xº@-•'ÎÏ0?þ E?z>`¿ÛôxÜÏh!¿àI€4ߛ¿Ú>«<7¿Ýï²!r7øAGNbllPKS 0118-272?ïü˜sU×?@±šô`?;ó<eQ9?@±šôn?ïàWÝVòG?y… ½,¤?o¨"©
º<?y… ½,¢?ï øCx»?—Œ›af³½?›à÷èœ^?—Œ›af³¼?íOÎW)'?°D©F^Žõ?µG¶Â?°D©F^Žõ3FGL J0121.7+5154@_ìÀ§¨À%_tÿ†]}À:›=އàÀ;—f=Kºé¿êz¸•)¿¹@
7¢wŽ¬×?ÿ¾Øà×EÍ¿éîÃà—´¿ÐåI=ê#þ¿Ò‡­rOº¿èƬªËúAGNbcuNVSS J012133+515557?ïÅÉÐqÒ?ÁÐnpÇú?}xÇ\?ÁÐnpÇú?ïQÊ»ª£? '¿©K48?•Æ¨œª«°? '¿©K48?ï+ÆÙ¢é-?–•R'že'?š‡$Ë¢Ú[?–•R'že"?ïänÛG?o¹Töxa?küç'$¹?o¹Töxh3FGL J0122.8+3423@`Hüàü.ºÀ<€ÌC:À9ò¯ñʳÀ;x¢?Zˆã¿ð–G²œ@
]Œ©ÇG?÷Áˆ`Œ1Ò¿ä"ÉÑ¿áÔ÷p0áí?°DS½¨}É?²žçóUAGNbll1ES 0120+340?ïýƒ¥-ùS?2S9Oߋ?3â֐5qJ?2S9O߄?ïê5הX"?q(øaÊÈÏ?eÊ(k§nC?q(øaÊÈÏ?è}
·?‰¾,rs"?à½R?‰¾,rsœ?ïÿÊ¿,J6?7ÜÄ[Ã>ú iÚäÔ¾?7ÜÄ[Z3FGL J0123.7-2312@gMó`Iì³ÀTmŽõƒ¥À9¤†ü#»À;ž_7ûÿ?͈–'ôø¡@'@'m€?ÿÐ1€Ö(¿êIÒ¿U¿É|ö«mŽ¿á©}~ÛÓ¿à+aé©ýAGNbll1RXS J012338.2-231100?ïúZ)îþ?G‰0Y˜w;?F—›XD	H?G‰0Y˜w=?ïè‡Ú[©?vŸK&ŽâO?gçx%¤U—?vŸK&ŽâP?ïŸPÿñv?"Z 3º?ˆ+À:C¢Â?"Z 3º?ï8É!. ƒ?†ø k÷Y?˜æÛÚ;ï–?†ø k÷X3FGL J0125.2-0627@b6"_õIÀPô'@.Ä9À:6¼ÿÐ/XÀ;×ÓãAƒX?ñGFÐôÏ @SU=õ"@©Ë€qt?ïj6&<D¿åĬ…%Ë¿æÇùG^'¿çƒ¬þPRAGNbllPMN J0124-0624?ïÜ!	ççŒ?|L±íÔ?qï{9°?|L±íÔ?ï¨Vìݚ\?–ùÍW>Ë?…êDșhâ?–ùÍW>Ë	?è¨aù÷÷Å?³LB'yw?Í^x  ì?³LB'yw?éòâm©?·³‡7Iîæ?Ëä4vIZ?·³‡7Iîæ3FGL J0125.4-2548@i ½ ßÞøÀT''?àÀ À:Œn7ìÀ;ãKÊíñ?ä)ˆ[òð@pÀþãJh@	läÛ¿æÉ "ì¿Ö±yJÕÍc¿ãPÎúyƒ¿çBӃdçAGNbllPKS 0122-260?ïùùƍ7g?Uâ–gØrt?HåË"fë?Uâ–gØr|?ïèæ.Öö?vžµ_?gÑ)ù
]?vžµ_?ïc+\~n¸?"qÙ'o}?"š"p2)?"qÙ'oz?ïdö&@?Œ<8.ýè™?žóa;=8?Œ<8.ýè›3FGL J0126.1-2227@g)Ÿ¡—ÀT6· ÝÞÀ9'r#3
ïÀ;§èÂ̙?æz–oÔµ`@Ĉ;Î7[@q'Iüο×:A؛Ì¿ä¹-ÔW8T¿ê˜mhÒì¿ä>»×S…ÛAGNfsrqPKS 0123-226?ïùÞp™ç?Q© ‰V ?H†?õ˜a?Q© ‰V­?ïð§©ò%"?g@ȸ<¶ì?^°¬´ù?g@ȸ<¶ï?íþò×î?Ÿ{»ÒŠ ñ?°ogi@ƒ?Ÿ{»ÒŠ ó?ïmŒ¸ø»?…HÉáøì?'Nhý è¬?…HÉáøë3FGL J0127.1-0818@b—ן#FVÀQWü€¿À9§¨Xy=ÙÀ;»ŽÐû«?ç¡J/¤‡@aé;îB¾@²ãàÈñ¿ãŸIÎD

¿áGk#|4¿æ÷Û\S
¿áNL•AGNbllPMN J0127-0821?ï-JŠõ?¡äw›ÚÒ¤?œ\Ö®¡ˆ?¡äw›ÚÒ£?ï˜$ölX?šõËoÕ>?‰öÂdéؐ?šõËoÕ>?옅ÁÙ?¬ˆ—1"?»;Ññ7o5?¬ˆ—1"?éKJ¢$(?´3^ä%?ÊÒ×Ýwo]?´3^ä%3FGL J0127.2+0325@aƒ&€IRÀM ªKÀ9LntQátÀ;hŒ'sZk?Þ8
(Lû@9rƒ«Ë?þce€À?ײÃ%	À¿àPxµÀ¹¿Ó҂4^g¦¿âÔWC~†AGNbcuNVSS J012713+032259?ïäÓ´Nñ–?g˜2°³"Q?k,K±jK?g˜2°³"R?ïÜGzJ±ì?w}}óæ?qÜBÚ§	è?w}}óæ?ï>#I—Ln?;ƒÃۓ#?˜;–Ír^?;ƒÃۓ$?´ô'(?'%+»?¥U¤°¶Ý†?'%+¼3FGL J0127.9+2551@`£ýq?ÀB%'Éä»À9¥Z'"ÃÀ;§YE³Æ?Û
ZÆõó7@­wt«¤@Ìc¿˜ñ¿çÃ&$Ö4¿ë涴BÎm¿ïÿì0€É¿à_ËÌ5'÷AGNfsrq4C +25.05?ïøß_\ëP?€ÑDI±0?L''ŒRÆw?€ÑDI±0?ï&xúbCÝ?±‹oï	U?›0à³·"}?±‹oï	T?ï	£jBÚ?"ÈΎÿŸ¤?žË'·¾dæ?"ÈΎÿŸ¤?ìÔs›£?³Ýç`ˆ°?¿y_"c"ê?³Ýç`ˆ°3FGL J0128.4+6257@_È
€CR?ÙØÀ1D,À8õeQ"qÀ;:-"wú?ì†ëÚ.4F@¯çcÑâ@	/ÿw¿àgÉ<õT¿åÕ=Ÿæ@¿å†ëabpŽ¿ïÿ‰OTHERspp?ß}!óÙ¯?ÐO¶ó†Õ?àAo"(?ÐO¶ó†Õ?‡šÿGî?–ÏkÀHý?ï¡û™"à?–ÏkÀHý?Ü–Ðu	t?¹Zmל>Î?áò4—Å{F?¹Zmל>Î?Æ€{å­¢?¦t±¯(JÕ?êzá"˜?¦t±¯(JÕ3FGL J0128.5+4430@`;ªÁ	J,À1݆ÀytÀ9ØÊUú˜À;Âٗ¶j‹?Ʀ/UÔ¦@ø|ôGe@¨À^Tt¿ã9\ZÒg¿ç™ë 02¿áۘ=_BA¿ë–ÞûðÉ#AGNfsrqGB6 J0128+4439?ïý=Pª$?8Ɂ¡OÐ?6uz®Öî?8Ɂ¡OØ?ï¸Dûˆ?‹ƒ-gǕ?ÿþîÁé?‹ƒ-gǘ?ï¦:t¿?…x@vc4?†qx¢ùè?…x@vc6?ïŶ?e;9?o%Ó51?}$àMbbë?o%Ó543FGL J0130.8+1441@a Ç`|ÀGšÿË&ÚÀ:5O•GûÀ;Â+,Ôta?éÈŒZÒñ@ˆaq´ù@4NŸö*¿àÁÄ¥®GH¿ë¿ì¡ÿC¿ïb…¤ÖIß?êal×n¼AGNfsrq4C +14.06?ïõ|{8?\é ×W?UÃåŽ{?\é ×Z?ïòZHê±Q?c¢8¬½3?[Kn*`d?c¢8¬½5?ìƁŽ‹n?ªj1J³Ö?¹Ë󏛤‹?ªj1J³Õ?ï˜aP"}p?˜É䓝‰B?‰ç«Úà¤?˜É䓝‰A3FGL J0131.2+6120@_ëğס<¿òµQ€¦-§À8w3¼ÅîŒÀ;§' Ö9¿ëëQÑ?3ƒ@êÍ–*y?ýÊ€¥+ô¿àÈSõlö¿â~zm?¯ª¿Ùq¾óŠ°¿Ìsì.›AGNbll1RXS J013106.4+612035?ïþ6—¡<?1ú+±I?/̖…ìI<?1ú+±I6?íb0Ÿòu?ÅӃ?Ùý?´î{lWM?ÅӃ?Ùý?ïyØn&Ã/?'5Ô¡zÉ=?Äò;'š?'5Ô¡zÉB?ïÿ$ÎÀâÍ?'këDJ?f'ã¦V7?'këD~3FGL J0131.3+5548@`οìºÀƒ<ŸÃFÀ:=0l¯VÀ;šºZ•¿ñ7`Ú5k@kÏæ1Í­?þv3þµ'?¿ëΐŸ‡¿Ý€Òõþç¿á#qKòœÀ?¢ÔoÁAGNbcuTXS 0128+554?ïùF5æ¤Â?Fªk;¿L@?Jç(elüV?Fªk;¿LU?ïmþ­©…?¥\-Âܳ?'@<êJÏf?¥\-Âܳ?ï•~)Cø>?ƒ¦tÃå)?Š u¯ð?ƒ¦tÃå+?ïÿégÏ?!ù©§sjB?ŸbÓ"	?!ù©§sj"3FGL J0132.5-0802@bûw µíÀQ%4ß۝JÀ:ˆÉûaÀ;¸A›«Â'?à :M·³@óˆzãK?üÚß_ ¢¿¶S"F@g?ïšÎãõ«¿ÚÎOT¦ö¿Ðà-ëSSBAGNbcuPKS 0130-083?ïø5h¡it?Qp=ÎG¯?O*]zZ03?Qp=ÎG©?ïé,uwQ?q;™HijÈ?fӊj?q;™HijÆ?ï6€Y¦èV?Ž®xÇÐÅ?™/ôË"õM?Ž®xÇÐÅ?î| ˓È?¡1Ž¬%y?¨=óFÎco?¡1Ž¬%y3FGL J0132.6-1655@ed@ò8—ÀSÁýaÀ8]à_PÈoÀ;Œ­Ánʹ?ïj
®ÀÙ`@홟£ÉÉ@pê¿üÚ²¿âðƒÑk¥¿æH @ÎbŠ¿éQØXNÔ¿â—!B¬BAGNfsrqPKS 0130-17?ïþ¥‹9?#Ûãzzbh?%®ÎWL_ý?#Ûãzzb4?ïóüä^æÏ?c +cq¬Á?X7B2aÃ?c +cq¬Á?ï÷"¬2¬?'ÈÙPK?œ
jyª?'ÈÙPK?ïÓçF"õ'?r°ƒ[mV?v\¶7¾?r°ƒ[mT3FGL J0133.0-4413@qy[À6ãÀQ½²_Μ±À:/ĦãÀ;üË+­-¿äP/5€H@@$³=°@?ü¿ÙŸC¿Þ jpX¤ÿ¿â~U<ê¹i¿àÈÇL/Xˆ¿äJ‡áò_AGNbllSUMSS J013306-441422?ïýôÛvK0?>'HÎÆ9?0Y$M¦?>'HÎÆE?ïñej›Ëª?gÜÔÙOg?]5*Èh©>?gÜÔÙOs?ﶭþ?•è‡ ïK?Ÿ©*_@2?•è‡ ïM?ïëäßFï?_ë´ÿGû?d ¹íw?_ë´ÿG÷3FGL J0133.2-5159@rˆv\ÀOö¸¿ÏŽHÀ:pƒÇ ="À;î£~éпÔâHæ_R@õö`X@kŸ`X¿êu«Èg¯´¿ã8c‡'Ç¿íÁ5
—±ý?ØJÛ~SÌAGNbcuPKS 0131-522?ïü´L¸Ý?@ƒ‰ª<"?:]ŸZ9µ?@ƒ‰ª<©?ïô
àŽ¦q?aÆü°A(?Wä>â³?aÆü°A(?ï7
+o¿«?Ž[£j²:
?™º'
x?Ž[£j²:?ïû"ƒ&??J-t"¿§)?A±óg†?J-t"¿§43FGL J0133.3+4324@`^œŸr÷nÀ2Ш߇ºtÀ:BЏ±¹À;Ԓr]ën?ÞÁ4]·ñ@¯ùO·£@h~€
¬f¿Í´›â&Ú¿éM$ÓknÛ¿áËÈ­zÄd¿æ9'%y-¶AGNbcuB3 0129+431?ïöéB7cX?Z8Xä…ð?R-{'9Pa?Z8Xä…ü?ïšHÄBÄÊ?"ì§ö.é?‰mÎïN͌?"ì§ö.é?îì[šèJ?•Ëf€9qr?¡8
FQ{Q?•Ëf€9qt?î²<µƒ©?ŽÃ0¨‹?¤Ü4§ÅnÑ?ŽÃ0¨‹3FGL J0134.3-3842@p¾àP7PÀR×"Àh¡À:E©¸ËŽÀ<jüY'¿è"íŒò@tM¿%šC@¦H «L¿æâ.ÝdÖ¿æÚešA=¿Ð·½å4¿ëøÎEGݺAGNfsrqPMN J0134-3843?ï÷8ydŠ]?f@f_/¸î?Q
6ëF)?f@f_/¸è?ï󢚋¾Â?cyààfâç?XºÊè'xZ?cyààfâä?ïH?ëm§-?'«ºÜ¡qÞ?–ø'KJ?'«ºÜ¡qÚ?ïûª5ö?A3»ºÏÁ%?AWÏ+¼&Ñ?A3»ºÏÁ3FGL J0134.5+2638@`׃¡	ÐcÀAŸT_Ó¥.À9bÒX'ƒÀ;{"qê('?ñÄmO¹¦ª@>¿Ä¦Ž?ÿÛg_4Ã×?ÑEÉïˆõ™¿Ù؀	O´ô¿ÝTžg½1¿æí¤èFÏAGNbcu1RXS J013427.2+263846?ìTæ0¨?¸yܵ‡?½X˗¦z½?¸yܵ‡?ívv÷u?·¡¼8˜<?´O§üHDb?·¡¼8˜<?çkÎW$&?µ§QÓ"Ñä?Ñ)ôcQ·´?µ§QÓ"Ñä?äIA:T=;?´1=÷û·?×m}‹W…Š?´1=÷û·3FGL J0135.0+6927@_°ÄŸ×¡<@¬Æÿ®K'À9ºGº©´šÀ;O‹Ëz½?½I¢z,°§@Ó.ö¸ƒ•@tcßÎ\D¿ÊIÅëKô¿ëÂsÊý꧿å¾ësè¿äU÷i"ªAGNbcuTXS 0130+691?ïžgàdKT?'
҇Ó?ˆfæí*ß?'
҇Ó?EK?´Ù6†Ø×¢?¤‹®+N	?´Ù6†Ø×¢?í¾
ð(T?©ÑÁ;¼­?·ê~½f?©ÑÁ;¼¬?íu:æÙ<{?¡ÜZéh=Ö?´V(É6.?¡ÜZéh=Ö3FGL J0136.5+3905@`9à`þHÀ6ñ§Ši{À7p͔ré,À:sˆ¬Œ%?çKÀÌþÓ@‡&°:?û!/à˜[¬¿á:p'2¿×ᾨ·¿ÒËjµ^#Õ¿Êþô^®ƒƒAGNbllB3 0133+388?ï¸ñ½Íq?†?Av‰šS?þƒŒ£µ?†?Av‰šV?ï´Ð-z~?¹»¼)è»?'Ëô¡`b?¹»¼)è»?쭆ø§?ªŠ÷ÙN—?º"Ï_À:Ä?ªŠ÷ÙN—?Ë$°"? !Áþ°Þ?§ÖsM´÷¼? !Áþ°Ý3FGL J0137.0+4752@`Yi ­ŠÀ,˜¥ÀïHùÀ7²MryšÀ;ªÆè‡=?ú"ç÷²@WK@î>¿àä-R.Ý¿ä¢jT¡[Ê¿ãùÁˆ(¶‹¿èãÅYÇ¿AGNfsrqOC 457?ïî$*`*?b8tßџÕ?aâÛ՟Õ;?b8tßџÑ?ïÎ?)c\r?ƒŽ 9$šà?xàkNQÆÁ?ƒŽ 9$šß?íüȁ¾@º?£'ötK$˜?°»ò
ú(?£'ötK$˜?ïúãé"N¬?Fô@2è?DpY®ÅQ±?Fô@2ò3FGL J0137.6-2430@i,ÀÒÇÀSÑÒtwÀ8柱mÀ;ÀØi¹>?ﯟ%°ÏÒ@ŠVf/]@$ Tä¿ã@ÎØk~¿çCAj¦¿éi¶¼Xû¿ç¾ãèÈ*ýAGNfsrqPKS 0135-247?ïþÝ•?%RùÑ^ôÉ?&"/æ¯æ4?%RùÑ^ôÀ?ïðˆ()?j–/-?_èﯭþ?j–//?ïm²©Ä?‡Íh¼Û-ª?']i¼
Ç~?‡Íh¼Û-¨?ïp(Äà ?Ž]ÝE¹#R?'úý'cü??Ž]ÝE¹#Q3FGL J0137.8+5813@` Ç1¾À\l.NÀ9Ý:ZMÀ;OZˆ%¿çê3!añÚ@Ü¡jHs6@u8_—ë¿Ú¶½Œ'¿äå?æ'šV¿ÞÁ¤G¿ÜO³7‹˜¶AGNbcu1RXS J013748.0+581422?ïä'ú"ª¶?gɗ…I?k}ÝUIo?gɗ…D?ï7œ²ºãO?§ݘ¨å½?™i¨£–?§ݘ¨å¾?ïg+œ%?"¯ƒ€ƒ'?žsœ,{A?"¯ƒ€ƒ"?ïè7ã!G?e㸝£ <?gÈÞð¹»?e㸝£ 43FGL J0139.9+8735@^ß/@_k @8ÇÞàˇRÀ:[o¨.‡ÓÀ;Óác\ƪ?ÎcJ]'@
èO-°7?þBŽ_Ô¦á¿î¿?97z?Ûd˜nSù/¿ã"=êZۿŬ†6́	AGNbcuNVSS J013913+873754?ï܍tšv~?uÓßI6Aƒ?q¹E²ÄÁ?uÓßI6A…?ï´jI¿{Ü?†åRL´›Û?'åm!	P?†åRL´›Þ?ï|-ïìÕq?‡Œ²ãžõ?zBeR?‡Œ²ãžõ?ï€l~Ê?"Η
'$?Ÿü²p&¡?"Η
'%3FGL J0141.4-0929@c╁$ÝÀQ19Ü>ZÀ8~ê–pÀ;Rùþ?ÜágfÊ@\ÀÃÕ@ûª ¨»¿ØòvÅf/¿ä1Q÷zÜ¿áh'N4§Ž¿ãÑi—H[ŽAGNbllPKS 0139-09?ïÿ*!fm‰?LøŽ¸K›?»Ó2N™Ø?LøŽ¸Kl?ïîꫳ '?iPÖEµ3?aTLßm#?iPÖEµ;?ﴁIáç?'œ¸{Ô?'ß­‡†Ë?'œ¸{Ñ?ï…ò±vBz?€æŒÈ?ŽƒS¢oa—?€æŒÇ3FGL J0143.7-5845@r'@$³>ÀLŠ+¿¡kÀ9)–‡å<À;h¦©L•¿úÊ+lë:Ì@ƒ§>ó±?ýj*þÜ>…¿Ù²ðm:ëä¿Ú`%¸)¿âðZ›ü¿¥Fÿæ!)AGNbllSUMSS J014347-584550?ïÿw']X?å6•–Ý?1
´TüÖ?å6•–÷?ïõ*Úß?`ã>ûmí!?UÛÙªJB9?`ã>ûmí!?ï€Aùɤ??4m÷s?ï¼Í–½??4m÷x?ïÿíÿke>éúXrCé€>â"ð›òü>éúXrCçC3FGL J0144.6+2705@a)  ôØÀA%ë`5ʽÀ7ÙcaÏ'ñÀ;a$WÎ?ò†¨ÀþãJ@D8"*@kïð=jD¿àK\øÜþ§¿ã_Š±
Bx¿âÕAVÛ¿ä —YAîAGNbllTXS 0141+268?ïþà߸َ?!=åœ?!òrg&ˆ?!=åœ'?ïÛPšø³ö?yÊ5P'w?rW²ƒ¦à?yÊ5P'u?ïPA¢€E/?'KX5}?•÷˯÷Z?'KX5|?ïNt×î;?"†š©|
?Ÿ–1e8w?"†š©|3FGL J0145.1-2732@k>àŸèh4ÀS"2_Μ±À8ŒpUÓq,À;«ô5Çb*?ñâçæٓZ@ýˆšBáÒ@Ž'`:'n¿äs'¹áÁ.¿çódÑfs¿èîÉëਿì(LQ"™AGNfsrqPKS 0142-278?ïñ¤' Z?WKmd¡°?]è¶Ú¿L?WKmd¡©?ïñhîðªü?gðü'€3c?]."ªØ?gðü'€3f?ï
µ‰Ï?"çµ".(‰?ž©NƐ?"çµ".(Œ?ïÈDäÕ7?t*³á?{ø]•dx?t*³á3FGL J0145.6+8600@^üá~4¹E@7<ö í¦À:@yꧩ'À;Ú|öË£Ø?ÍÏ·úKO@e™
©@&«?ß>¿åL{7-ê¿á¨å¨P¿æØþ"¿æ¦_&oðAGNbcuNVSS J014929+860114?îÆ °É
-?¬RÞöòم?£ôóo]#?¬RÞöòن?íÀÞvTÙ,?µNìfß3l?±ùMY6¨?µNìfß3l?íóoÿQ ?¢o‰*Îw?°d€wÆû?¢o‰*Îx?èœ[Ó-(½?µ²¯õݹ'?͎³K]
?µ²¯õݹ'3FGL J0146.4-6746@rqú?̞ªÀHB=ÀTïFÀ:4Ò{bvîÀ;÷õy"@"¿èzjÉfT¸@
ÂPŸªª¹@ )`vP¿ãµ¡Øà׿åFGž¿é=uó»è¾¿Öb¤æåãÛAGNbcuSUMSS J014554-674646?ïõ®òO?Xµ_a쫁?T£ßúd?Xµ_a쫈?ïïcRr؅?lK~G	?`œ­'zä?lK~G?ï
¬\'¯õ?'å‰`¤À?žªtmÊf?'å‰`¤Á?ïò‰jø?X—"ÎÃè?[Òí*àß?X—"ÎÃö3FGL J0147.0-5204@q¿?á—_ÀOz-K6À:=ƒJ¢»À;þ0íÖ¿íÊ֗?»ñ@:9/K@˜¼ R;¿Ä¢¾lô¿âð³¡á¿ç†kEÿÀ8
{Œ›ãAGNbcuPKS 0144-522?ïÕ7<cZþ?†…•^‹#œ?udaÎR±?†…•^‹#œ?ïöH~ÿ¥?aniÝI?So´çæ?aniÝC?íéÁ0©ôk?¥í'Íð™ø?°±öz°\²?¥í'Íð™ø?ïþ¯wg¯?.óoSÝ?/µ‰"ÿÓ?.óoS¿3FGL J0148.3+5200@`xwß (À#Ä9 1xÀ9¸þ›{ñéÀ;%îÇÉ?փՁò"@cFçp?üRóÀ+©§?ïýìH#k{¿¿Î'¢À¿ã¢+e"]g?¥©yámmÂAGNbcuGB6 J0148+5202?ï÷Ùåá×y?QëO…l·ƒ?PL4<Q:?QëO…l·?ï2®ÎϒM?¨YjÈ("?™ª&&
¶Y?¨YjÈ("?ï	UÞå)?"³Z¡?žÜõD#ZÜ?"³Z ?ïã!w‡'?fn`Ɵ'?lވîxmù?fn`Ɵˆ3FGL J0148.6+0128@bÝ"ß°Õ ÀM †¿¢AßÀ9ÀX·Q:…À;ŸŽ'å".¿ÙXim×ÉÖ@†öA»6L@*@\fˆ¿Ú³ßæ…·¿æ—Oß³§¿Üvpd_¯¿Â•Òÿ[AGNbllPMN J0148+0129?ïÿÍm¸(>ôÕ 
¿%>ùI#ëûò>ôÕ 
¼ß?ïó㚕¥-?c_Ú?X8ÊÔµ¤´?c_Ú?ïڊŠ–G?uK©D§»o?rºº·´Üƒ?uK©D§»n?ïþcmE¾?#-Ÿ'ë¶\?)É+§+	?#-Ÿ'ë¶l3FGL J0150.5-5447@qÚ®_ú;›ÀN(}?Æ¿mÀ:ÎakTâ°À<*'ë"z¿þøYÐÖÇ¢@CpcÀCÒ@ò -1'¿íïÔ.ž"¿Ý¥Zõfkf?aBàÖl«¿è2£Ý¯AGNbcuPMN J0150-5450?ïÏzM©W?Š¡ŠTv7§?xBÙ+9Sç?Š¡ŠTv7¨?ïôŒw	?fßá/×l?Vzçïí?fßá/×m?íw)²äþ?°o°S~ ?´F²hې?°o°S~!?ïÿÚTÜkb?xŒ÷ÄY>òՑÊNÊp?xŒ÷Ä	3FGL J0151.0-3609@oƒÿŸ‡ð$ÀR†À
¡©À:mtòd/À<gpQ¡³Àæl¿@+-']¶@¬]·ñ¿çųT
{¿å5m:ž•
¿åžçsŽr¿Ö"½.t1«AGNbcuPMN J0151-3605?ïüxÑ
¹Õ?E¤@WGÒ?<9wª1X??E¤@WGÝ?ïõ쉱Ç?bvÔCrُ?T'èìœr"?bvÔCrى?ï8–œŽVj?ŽÒ,oäÇ÷?˜í,n52Ñ?ŽÒ,oäÇ÷?ïÿú"Áµ¢>ÓïhYÊóó>Åìù)p½Ÿ>ÓïhYÊô†3FGL J0151.0+0537@bœ] l‡ÀKK¹ëÀ:o¢äßÀ;Ӓºǿޔ®tl}@
w¼'&á@@ߜÿªšž¿ë<TÞÕ¿âA¾¦:ß¿ßlsñTl¿à÷ŒŽ™5qAGNbcuPMN J0151+0540?ïý÷$yœ?1™'ìÁM?0GÖÜ3é?1™'ìÁY?ïñënÎd?h:i¦‡ñ·?]Ð)"c8?h:i¦‡ñ³?ïOü¨Œeþ?''o`¬o?–jîs@?''o`¬j?ï窩ªC¦?_bgvgÔ?hUVU¼Z'?_bgvgá3FGL J0151.6+2205@aœ~`Ï6ÀCU˟¦#À9½#nšÀ;º£ø'Ä?áÄDã‰Ò§@š§_Tú-@;[áF׿æÝÓG7p¿çݶÂs¿æœÛàæà¿ïÿ}¿|AGNfsrqPKS 0149+21?ïØØs¯°·?}2ƒ¿?s"Æ('£‹?}2ƒ¿?êý¶:pëÐ?ÉTêŠP€?Ä	'<PÁ?ÉTêŠP€?:+'?šijl¼÷Ö?¦.ÔÌ]Fæ?šijl¼÷Ö?ä'`>xÁh?·Ÿ*dAÂ?×±?ƒ}0?·Ÿ*dAÂ3FGL J0152.2+3707@a
¢À8+À~à±À:>'d@ò9À;ârÚ/­¿Â©—âùùš@&¶£Ã@@vÀP½ˆ¿Þr²™3±ø¿ä®K×¼6t¿åˆMD+~¿å–IÕ$ùÎAGNbcuB2 0149+37?ïºú¬Ôz©?‡+¥º?ATÊáUö?‡+¥¸?¦ÉÃÉ?ŽéÖÁÉã?€ù͏
¢?ŽéÖÁÉå?í­€Ûv"
?¦™ÀN›©?²"ù$KgŽ?¦™ÀN›©?ïnñ¶'‹Æ?',¡QCOe?'!É-®‡i?',¡QCOe3FGL J0152.6+0148@co€UûµÀLÃ)ßÍZ'À9qè
šó6À;rÔ#&v?'¤ŠŠô?v@'˜ª†Pç?þ/žÉ.]¿ã}ûüþ¿ÎU²;Hwà¿æ1ð\7Ó¿—TŒQæ_AGNbllPMN J0152+0146?ïÑëëçD?xÙuJìê³?wz

^c?xÙuJìê²?ïñl
Òvþ?fÒ©Â_?]'ä[#?fÒ©Âd?î/¹8}À? Yxî¥@Q?­l~¸#û? Yxî¥@O?ïÖæ5¦î?o®ßa L?tŒ¸e,‰?o®ßa G3FGL J0152.8+7517@_¸Ôýó¶F@)ÈÒÀ+ԚÀ:–›¸WËÀ;±"Pª<?ï¤ãŠå‡ë@1­@˜?üS ?ïD¹®j"§?£«ÁlúÞ¿Òò-¬-}¿ÛZâÃÈÛëAGNbll1RXS J015308.4+751756?ïâ½g;·"?qáGZ³*?mB˜ÄHÝM?qáGZ³*?ï˜ay™ï9?'Óp&ɯ}?‰ç¡™"2?'Óp&ɯ~?Cð	6?¦~ô»¦?§ÇÀÿl™?¦~ô»¦?íV¦œ(%?¡Ê4{Ғè?µJËf¾Ñ?¡Ê4{Ғè3FGL J0153.4+7114@_ûÞ¨—c@!òU¿û?À:Fó½Ò^À;¢nfåè'À›	º"å%@ÎkéG'?ù~àZÉ$?ÙhS.-î¿åVüæ¿Í$Àdð¬¿Ð¡}ÇñØAGNbcuTXS 0149+710?ïûƒü?C&Idt?Có»'ð
H?C&Idt?ï×U'7Äk?‰ÛÐÂÀ??tUldÊ·?‰ÛÐÂÀ>?ï‰âl?EÕ?…ÖòÖ1'M?‡dð.Š¥?…ÖòÖ1'K?ïÿå?`NQ>òE'è¤m>êÀŸ±®;&>òE'è¤oi3FGL J0154.0+0824@b‡…À3aVÀI® ö½À8)+rt'À;
ú滋\?ò…­¶Üöf@¯í|Å£c?ýÀ(~ú1	¿Ç'ދ'A¿ÞF²ZÊ¿Ó=ЊòaÝ¿á>qðˆ=ÒAGNbllGB6 J0154+0823?ï¾I> #?…zû¤ÿ?€m°wü÷T?…zû¤þ?ï©Ï4R5?"€‡7CR?…Œ2ëzòÈ?"€‡7CQ?îöøJލ?¢P˜SáÄ?¯€{R?¢P˜SáÄ?駇Ós‹<?±)@>¢`?Éaà²1Ó?±)@>¢`3FGL J0154.9+4433@`Õø@À0Ý¿Sg†À:_`¸§|À;ÒËÖ,Çß¿÷1ϨÊ9@f.fš¾³@w€ KÏâ¿ÞzùWf¼¿âÕ
Ý}
¿è"õïʗ'¿¸b
CVÅAGNbllGB6 J0154+4433?ïëV(ý"?q'Ï3âc?d©×äj…?q'Ï3âc?ïÕ~³Pí?'GÒŸˆÅ?u@ò&WŠ?'GÒŸˆÅ?î~qŸñ4? WU-BÅE?¨ïöìæ? WU-BÅE?ïÿ՛ppË>ú†jqÝ[Ç>õ2GǛ)>ú†jqÝ\º3FGL J0156.3+3913@a
Ô2TçÀ5î¬_nû`À9ƒL8½¶¯À;Ë+/X³À¸ûh¾@(³Ä"t@öA?»VÙ¿åŠXµ	ð¿è_Pé/6­¿à¯öäV	¿ïÿë‹åãAGNbcuMG4 J015630+3913?ïÿ7§ ¤?†ÆÁú~?²7×P?†ÆÁûn?ï猊òDF?wËÈXMsÞ?hsu
»º?wËÈXMsÛ?ïÁ׺°&?}†;Ï©9…?"§ìóP?}†;Ï©9…?ïÿþ«ûx'>Àrì6»>¥@HwÐ3ò>Àrì6"á3FGL J0156.9-4742@q6`ÀiçûÀPp×?íUÙÀ:õ©ŽÚ"÷À<&¬k-v¿ö¹Ô,g'@†Q
^¨­@¥ßx "?ü­–‰¿ïiŒFR}Y?ä(_ÂÞ6'¿¢·JüÊã¶AGNbcu2MASS J01564603-4744174?ïþƒ$MŒ×?;âØLpo?'Í»'2"´?;âØLpQ?ïó&Cï¾?fxv5à…?Y³x!ƒS?fxv5àx?ïï'FN?–öH±%%˜?·,VR?–öH±%%™?ïÿüäCÎf>Å]r7E´2>¸ÝáŒ×Éh>Å]r7EÈÆ3FGL J0157.0-5301@q¢ß?–ÀN°ŸõÔ-À9ž´À;(Âz?ò¦Ì,¾Ïß@Œ,ºÉ1?ý*
h¦?ÛM{'ƒ·¿¾x9cN¿Ì5¹åg¿æ WÊ}AGNbll1RXS J015658.6-530208?ï\maóP?™Ãà£×g?"rSÁ•ø?™Ãà£×g?ïª
_?†ëÖåèö«?~þ*ù~Pg?†ëÖåèöª?ëÁ»À5?ªóEÆÏd?Àûë™ÿ,?ªóEÆÏe?í´qáŸ?§N)x°¡µ?·ß"\pó?§N)x°¡µ3FGL J0157.9-4615@q
?ÐÐhÀP²uÀjÀ9Áj©ÂÉÀ;çl¸ÿ?ðÎeä¶@H'"Í.Ç@˜[À6ã¿ÞôË·"ž¿çœû7昝¿æèf">®¿ïÿëÆj»"AGNfsrqPMN J0157-4614?ïĨ(÷H?'ƒ°ˆÝ Ž?}«ë"[õ°?'ƒ°ˆÝ Ž?í˜1–³?¹=¼AÎ¥ñ?³>sK—2m?¹=¼AÎ¥ñ?ë_òÓ¾2ì?¯»¿hÄ{?€4±4P?¯»¿hÄ|?âî¬gyAæ?»ëm10£Ê?Ú"§1
|4?»ëm10£Ê3FGL J0158.6-3931@p,Î?þó'ÀQÔÀ_×,À9XŠÙã5ÅÀ;Ã¯Ù`?ÞÖæü£Õ@ë«/™Ì@.HÿxE·?q×U¼Ê÷
¿ávþOž¿âÅ
¬N¿Ù»+ÅUµAGNbllPMN J0158-3932?ïþHŒ¦Ð?)²ç=¾%?.{w5"?)²ç=¾?ïðÝÝ4Ãæ?hr2í?^DE–x1?hr2í*?ïqNÆ­ys?‹Œ6åO?'Ö'*Pх?‹Œ6åO?ï•6ž¸‡«?zDÖÍåW¹?Š²XQÞ\?zDÖÍåW¼3FGL J0159.4+1046@b–¯ÀL‹ÊÀHT(?º*3À9MPíX]À;€¯°î¿Ð	'û%áÍ@Ê#EÕLM@èHÞ½¿æ=ô$™V¿á©'¯èˆ¿åãtó·¿ÇÃ\ôÖ3ÜAGNbllRX J0159.5+1047?ïú
ï Ï?Càˆ(Š¿?FÈC|¿
?Càˆ(Š¿#?ï󳅡í%?d"{ŽdÌZ?X˜ô¼%¶U?d"{ŽdÌ_?ïZEe%,»?áƒ"Û 6?"·S[ZhÄ?áƒ"Û :?ïó¶®ÁŽö?Re=¦m‰ý?X'¢|âû?Re=¦mŠ3FGL J0159.8-2741@k`–óEÀR´›€#¦ÎÀ9þ¹=£ÏÀ;ضXí ?î!J˜]7@Â5'ÿùJ@JIÀ4¿ÓdTªô'@¿Ó§¨Ì£˜\¿á-=…œŒ"¿é~"لý<AGNbllPMN J0159-2739?ïlûÔ¸¿?››á댳?'`…hýè?››á댳?ïÁ|šÓ?Šö!Ÿ€Q?~Aü2–?Šö!Ÿ€Q?é–AL¨ÆÉ?´x?|Þ»?ɦúÍ\äÚ?´x?|Þ»?ì'zJ§Ím?¤M$|2×?»t-ªÁ"?¤M$|2×3FGL J0200.9-6635@rGÆŸ¸ÀHñ7À:/œÔ·|ÙÀ;ñò¤ÍªB¿ï)÷é00@î#Ž¥u@¥ Z¨î¿ãµ¹óA‰¿äÔÂâ4µa¿ç+À"‡b¿Þ(>Ã4G°AGNbcuPMN J0201-6638?ïþxf"úž?2ŠÃÅÌâ?(y–ÀV$g?2ŠÃÅÌÝ?ïó?µßÌG?e#âþ4"³?Y€"@gr"?e#âþ4"°?ïŸVªt.?"(ßLðV"?ˆ*Ubô{º?"(ßLðV€?ïþÛ(w[?,I"rEµ?/âMxŠ:k?,I"rDþ3FGL J0202.3+0851@bݍ`¦3ÀI/ÿ¢/À:€\GÿsÀ;ÕiŠÞô?ï+Í+þqÇ@
=`'@as\f³?ïÿ—›UÊ¿àZ¦íÈ£{¿à¯€`¸}¿éo~ýOæ6AGNfsrqTXS 0159+085?ïz¤:1Ξ?¥e\š?«x¹Æ,`?¥e\™?îÏ~­78?§"š&¶?£,Œ™?§"š&·?çÆwISVÔ?¹!:
QQ??ÐsmYRV?¹!:
QQ??å:1‰ð_?¸³Wæ»÷?Õ‹œìC?¸³Wæ»÷3FGL J0202.5+4206@aԀuÀ2Öÿ_ÇôÀ9臢 PØÀ;ӗù†i;Àת´*8@z*ßQ´©@4JŸá\Q¿æñO:þ¿æêPé|…ã¿Þ#q_Ïڅ¿åíTW°@AGNbllB3 0159+418?ïÿ3`Í^?ÒH:èí‰?"îT4?ÒH:èíŽ?ïÞFSMß?~@‹r?pò\ÖY'?~@‹s?ïÕ1îÚ8³?vÞ'"œn7?ug'ã¦?vÞ'"œn*?ïÿýZü
">ÆþCYúÁ>µ("á6w>ÆþCYû´3FGL J0203.1-0227@drä¼®ÀMøK¹ëÀ:hØÿ
6»À;ðL'8¿ö+?(´Õ	@ُ'Î@€Ÿ¨Qm¿ãÝêŸÛÜ¿ãÂ73&¿ãJ<ɦ¿íǔdâ"AGNbcuRX J0202.9-0223?îQåËðÖ7?®
ò(Êz?ªá£@òœ"?®
ò(Ê{?ïñj±½*p?då±|Öµ-?]*œ…«"Ä?då±|Öµ+?쫍É–?¨S3#?º£'·ßKO?¨S3$?ïùÞV̶ª?J'€káæ?H†¤Í%Xî?J'€káæ*3FGL J0203.6+3043@a™Wÿ›V2À=¢ê šª;À8Ký¥²¬À;3˜ÿ?æ ?÷ÃkQݘL@†Êò9¼?ÿ?Ü+zÝ¿Ô\ãÐõPz¿ä+y@nì¿äAÜÕiº•¿æ{¬F‰@AGNbllNVSS J020344+304238?ïó¥GŠÖñ?_Vqç†Ü?XµpêR3?_Vqç†Ø?ïíN0×
?jä<ÉnyÀ?b±îÏ(òï?jä<Ény¾?î28ƒ!œ? àÎç-ܽ?¬ÜwÍæ?N? àÎç-ܾ?ïÿ*è^A?˜ƕ´^?¾'ô7£Ð?˜ƕ´½3FGL J0204.0+7234@`î¿eÛý@$ô "AÀ9-¯d9ÖÀ;aâÔvz¿ºýŠ*¡ûN@,F|ç_@ÅÈÿ¿F¿ÙnQÂ?€¿è‹ÌŒ¢å¿Ü©ÁÕwì ¿âê%Š(8AGNbllS5 0159+723?ïô'=ôÅy?^ޓe"
?W±"u¢?^ޓe"þ?ï¬E'rü?8,¢—t;?"øA+?8,¢—t;?ï-Øyؼ?'À—²ÖÔï?šDðÄýÈw?'À—²ÖÔð?ï˜Hpb×Ü?ì˜Û‰3?‰íãçJ	4?ì˜Û‰33FGL J0204.2+2420@aí" ³Ô®ÀAΓ [TºÀ:ÑÊbAÀ;șÌÅ@¿Ê/'Šxá¶@
Óú=ž?ü­ŠÒS?ÕÛç·èË¿Ú."f\‰¿âÛ@°…€?´ïA8P÷AGNbcuB2 0201+24?ïûÌyïÇi?EVÀäòüK?@Î@âaE?EVÀäòü;?ïð9ˆ|¨?hN""æ?_Œï¯ÒÌ?hN""å?ïXsÀcVž?‹±eø²Q?"ñ‡ó•,6?‹±eø²T?ïôœ';?S¼Aà!
Ø?VÆà݉ÁH?S¼Aà!
×3FGL J0204.8+3212@aü–þµÀ<%»À5ÖÀ9F	ç	ŽõÀ;åŒ·3?ÞÜ~¸@!↝h†@Ž—?w9G¿èð+Ña~m¿èz—U'пïÿì%úÝÏ?ïùqæ¢5õAGNfsrqB2 0202+31?ïù@ÏR	i?p‰;c¯Ð?Jü·ÚVÜ?p‰;c¯Í?ïæ*&' x?|ÊbŒÏh?iÕÙm߇H?|ÊbŒÏh?ïnii:?‰ÀÚ¤ñ€÷?'2ÜRÜxª?‰ÀÚ¤ñ€÷?ïñzí†õá?g¾"nn¯…?]
$ò=D?g¾"nn¯"3FGL J0205.0+1510@b€ºÃ.¾ÀF	՟Ú%{À9M­Ûoý¿À;¦G'ܾ¿ñv8;/ÖÝ@± üÏÊ@= v­†¿æ•'¢)`¿æzò@"‡Ë¿è*…ŽŽ'n¿æt=IaÕAGNbcu4C +15.05?ïÿ86Êg?``Å]9³?ù?¦³0ü?``Å]9·?ïów°Ñº^?dÊÛÀeA³?Yž\‹Eç?dÊÛÀeA±?ï½.~ôÛ?x"d
–Â?€´`BÉ:§?x"d
–Æ?ïþ²IgâÆ?&2¬Äú=r?$ÛiÓ')?&2¬Äú=e3FGL J0205.2-1700@gB¨€QÉ÷ÀQ‰ÿ`2o¿À8ºyà–®-À;¹C'&?ëÉîóµ'>@F‡7¯D@c¿Âù¿æ»§[¬¬¤¿éËÄOr&¿ìÁ®Û¿ïþ%Õ|ž·AGNfsrqPKS 0202-17?ïýÊëŸ?9·z,'?7灨£q?9·z,'>?ïò8È\Üú?hwC‹È?[ŽoFF
#?hwC‹Ç?ïbïy}z?²"Q©E?"¢ސP?²"Q©C?ïÙJD J?nÃhø?sZݯÚþ ?nÃhú3FGL J0205.5+6448@`VþKZ@£ÿywÀ7¡Û§[#<À;»·Ñ"?ùhÎÆ!7@ú˜Ê¼§;@¦Åæ(¾e¿àƒQé3$¿äŒ–EYÚ¿çè-µè&<¿í
9äI¸}PSRPSRPSR J0205+6449?fo<ðv?p4´ó:PÓ?ïéøÃü?p4´ó:PÓ?Z•…"é?~°wô¯BL?ïòµ=|½ž?~°wô¯BM?¶ö)go7?§¬²d$0ý?í!:Ó?§¬²d$0ý?onۄÏ\"?iÿ9¬Zú?ïà'${0¤?iÿ9¬Zú3FGL J0206.4-1150@eóWŸ#FVÀP¬Å@'HÀ9Z&d׍À;ÄAvÂÔü?²dŽPvv:@Gµpå›P@¦½M¿ãºÞì<²¿åRÙr2ދ¿ß¸ôäÕ}¿ëM‹,T­èAGNfsrqPMN J0206-1150?ïþqV¶¤?,kÞóÌ	¿?(ꔟ¥°?,kÞóÌ	b?ïõg{Ÿð?b~ÌÑHH?U1	úÀö?b~ÌÑHG?ï'½
¨y?‰©–fqÄ?y¼•áp?‰©–fqÃ?ïÿŽŠ¸2?	oJLÐ
Ÿ?]Qøó›Ó?	oJLÐä3FGL J0207.9-3846@o»'_ét£ÀQT_Ó¥.À:,x'¸ÔÈÀ;ü6'cDs¿ÔýÃw"@÷Îú¤vl@Zk@•ÇR¿ã[c$VeV¿é&çx¨:û¿ã¥¯½ƒ¿ì	i4àeAGNbcuPKS 0205-391?ïúÕ7'«?Rå¤Jí?Gð«!¹VA?Rå¤Jê?ïìÃ:Ot1?l+ï¢Ïl?c<Å°‹Ï·?l+ï¢Ïh?ïW '[³?Ž=À£®˜?•þ
ԉ˜?Ž=À£®˜?ﲿŝ{?yZ4Aä	?ƒP˜¡?R?yZ4Aä3FGL J0208.0-6838@rMÀÓgÀGy¾Ÿã_¶À:	~(úË
À;â½µÔì¿ÝÌǗ6pˆ@ÞXºla@]HÀŽ%¿ãâú˜ž¿çZ|Oz£¿â"Œ c¿æKõBÑz AGNbllPKS 0206-688?ïù	)˜Ö"?SBN'u?KÛYœ¥·œ?SBN'y?ïɺf*Æ?‹²ìÀçU?{"üÌêœS?‹²ìÀçU?ïVªíœ`#?Ž×¤¥Ù®…?•*¢Lsûº?Ž×¤¥Ù®?ïl'c@â??‰(þ
2œ¡?'mӗã¸D?‰(þ
2œ 3FGL J0208.6+3522@a‡?'æGÀ8á݀y7$À:v¦—®ÝÎÀ;¾Â±(,¿¶ÄY'À@
F¹q?ûG޻⚿ïÿæƒhf?ïü™¬l¥¿ÆFóƒN¿Ý|æì™×éAGNbllMS 0205.7+3509?ïü‹yŽš<?;XN¶êK?;¤3‹.#»?;XN¶êq?ïÉ>5z]µ?…~9d"á?{`åBÑ$Ð?…~9d"ã?ï· IðsÒ?z•zó×ÔÚ?'íƒãK?z•zó×ÔÖ?ï¸k?W?w‰žKü{õ?~£Ê`vSü?w‰žKü{ó3FGL J0209.4-5229@qeˆ`VíÀN_JÞ™À8"Š¥àϹÀ;¤TÞ¿¸ýûh@ꨍþ0?üÊÈ`Ví?¯'®\¹Y¿á#}ë麿Ð*.QÌüH¿ÜàÏT!ÑrAGNbll1RXS J020922.2-522920?ïÿ—Õ»N,?	ë õš3?

',tú#?	ë õš2E?ïñ芌È?gûW›w?\.êçÖq'?gûW›v?ïÝv{XßW?sµ[)á?qDÂST?sµ[)ç?ïú#Ëì"<?Bx"ësHá?GpÐOw¡?Bx"ësHÓ3FGL J0209.5+4449@a&uûmÊÀ/Â\ÀË6ËÀ:BÖ?<VÀ;ÒØ|-x¿ä©gög¡@Ø j™&?ÿ'DÁ%#ѿ߃õK$¿éw";ueÌ¿Õ²«·1Æ¿Å͚xÍØLAGNbll1RXS J020917.6+444951?ïÿ‹Wï?
Óļ÷¾?
*À;Q?
Óļö¼?ï×öMÑã?»É6?tÙw—?»É6?ïÎþ ×Ö?y <gªyœ?x€¯"öÀ?y <gªyª?ïþŠ©ÄÓ?"á=šì[?'^c²ÀÁ?"á=šì3FGL J0210.7-5101@qAÉ 'RTÀNâD?Êñ*À7²¢
¢À;5ʎ.+Œ?øêò4:o=@úJ´Y9@»zú;¿ât}ŸÔÆ¿ãÛb¥þ¤¿æéãC!¿èDUºœž‡AGNBCUPKS 0208-512?ïôŒÇ4Å?V˜ë3ÔÓb?Wðæq–yÚ?V˜ë3ÔÓl?ïõŠ˜d?b¯»] ?UðëæÏ5Í?b¯»]#?í×s­ê^ê?£ž>©Oç?±Db­«?£ž>©Oç?ïÿrqŠ²?
^~։w?±Þ.©Ùõ?
^~։3FGL J0211.2+1051@c}sÉÀG®ÀGƒLÀ7Ƨf
öÔÀ:ì)é•ö?øf)Kf†@4ïY¿Ž÷?ÿU¥`ÍX¿Û\™Õ9éí¿ä1øh1οà÷[s:¬œ¿æ.â톼ÙAGNBLLMG1 J021114+1051?ïü÷]ë?:¼ûœ¿$?8G¥€—'?:¼ûœ¿$?ïòf">¤í?fzcþÖeD?[2ׂ¶%T?fzcþÖeB?ネKL ?•³ºö_®¬?.ö–l?•³ºö_®®?ï÷ €Wâ ?N‹Ã#?P¾ÿP;Á-?N‹Ã#ñ3FGL J0211.2-0649@e3<`ŸÀOI¥ÒÀ:wò
ÎõœÀ;ò¼.ÿ?ÒIWMöÁ@ÿsì@Ë·À A¿Óì¿þC¿àÆۘäà6¿ÓYú6+Ný¿î‹o5~"VAGNbcuNVSS J021116-064422?ê`jnÜð?ÆŖ>Ó?Æ~VG€ŒB?ÆŖ>Ó?퇣€ÊW?À®~?³Âãÿ¹­T?À®~?èõ½¢4/?¶dA¶¤—?Ì)w/??¶dA¶¤–?ìÐ«ê:*?¯êÑHÖ/ä?»'z ®.¸?¯êÑHÖ/å3FGL J0211.7+5402@`Ԙ€"åÖÀô'€—†À9¶^®@¦À;DDЩ*¿ü^øáӚ@
»Õtç·@‡¼à²^¿æyüàÎü¿é´¡¿¥>`¿ædŽŽ½ad¿çŒ
IYAGNbcuTXS 0207+538?ï¼@5jÜ?¨¸@?€ïò¥yÔ?¨¸=?ïNú)éga?°yÛÑø}¢?– ºÂÓÚ?°yÛÑø}¢?î-Ó,Çô?Ÿ.0A63ð?­"Í3€¿ž?Ÿ.0A63ñ?ïü+(øuA?F¦·rp™O?>¦¸<UêÔ?F¦·rp™G3FGL J0212.8-3504@nOЀ¶sÅÀQ¹¸!ïÀ:f°8AÀ;êTà,%"¿é#äV‰Ø@rå$ÝZ@ã矋öï¿Ë—pe~ñ¿è½VÃcË	¿Í'$[:¿ßdGKݽÐAGNbllRBS 0292?ïþlì™<Ÿ?8‰eRš=ü?)16l6?8‰eRš=Û?ïõr›ˆå?aµ[¦íV¦?UÈî5ÕP?aµ[¦íV¦?ï•^¸{)?‹aeX×Ì?Š¾(Qá5ý?‹aeX×Ð?ïþñŽô?#¥¥ürÅÃ?' æ÷¶À?#¥¥ürÅÖ3FGL J0213.0+2245@bN¶¿DNÀB,Ì?ß À9L=Ÿ¿™À;ƒ*¯ÖòÀ¿ø9§v@ò3ä‰@Éè <öÖ¿ØɄ\µQu¿â\û"+7ß¿æ'Y=çtÌ¿Õ$olZ­\AGNbllMG3 J021252+2246?ïtL×¾]^?˜Ï%æÒ?'ve4T.?˜Ï%æÒ?ïìîÆÏ_h?pZP¸W?c90 –½?pZP¸S?íeb¨?§ÖñЩ'æ?·§GÜÔê³?§ÖñЩ'ç?ïý΃ ÈÏ?2ü'¿Í?1‹âù¹Žf?2ü'¿µ3FGL J0213.1-2720@kJµa
ÜÓÀQöÛÖÀÀ:ØU½¡¶ŸÀ<†Ï'yë¿íòcއñb@òSDÀ@µ­S·ã¿Ë—$¹¿¿éª"‡Ð³%¿Ýç'/xú¤¿º)¸[â»AGNbcuPMN J0212-2719?ïûxÚ7ö?kïz"þ)v?Cþ— +±?kïz"þ)x?ïö±>¿Nä?`'4ƈÀ?R'b7ê?`'4ƈÂ?ï&-Ñ«v1?•Ï¿¾Ìz?›:Eʑ:?•Ï¿¾Ì{?ïþ}-fò?$WŠxÒ Ù?(-/‰Ù?$WŠxÒ Æ3FGL J0214.4+5143@`øÈS'^À""Vßà¥ÈÀ:'º'GmÀ;²B@p…?Ýóõ°›¾¸@ӈþ–É@Uü?V,2¿ì=b\I4°¿íeÈ9ü6X?ä)¡¢¾Ë¿âp6,·ÄAGNbllTXS 0210+515?ïý¿Ä`?1fx)6ž?2áÜÿî‰?1fx)6–?îø¯òmóè?°ò~€7°? uÙ Án?°ò~€7°?ï²ç…Z?ƒèÖ3³¤?ƒ~†8©Ý?ƒèÖ3³Ÿ?ïârrøÎ?…âi
?m䍍3Ú?…âi
!3FGL J0214.7-5823@q»O?Ù3ãÀKØ'tÀ:MvÁ'}À;øшp¿¼ƒõÃf@ÿ/[bQ@O@…Z¿çs»
²›¿è'Í–ð¿âµpŸÐ?s¿Þ*x™Ä·ªAGNbcuPMN J0214-5822?ïÿ'ßz£Ž?Ú{¾h"_?H!WDõ?Ú{¾h"=?ïñá¦LR?dr7#_·?\<³g[ñD?dr7#_·Œ?ïÑVas&×?v- Y+þ?wTÏFl"®?v- Y+þ ?ïÞ|Ξ!?d¯
êÉ"6?pôA˜°ïð?d¯
êÉ"43FGL J0216.1-7016@rO}ŸÓo~ÀF—€"ØÀ:)ݨ½#À;äsùÍ¿å²Åz'ƒ@8"IÖã§@…A¯ó£¿æä""Ðÿ%¿ç­ëè	Øá¿ç:dUr«Í¿ÎaßÆ$@AGNbcuPMN J0215-7014?ïýLë°@#?6(¬œ"+?5˜¢}þå¶?6(¬œ"?ïóQ†7)˜?c—Jiç?Y\ó'¬Ìä?c—Jiì?ï‹d2C•½?ƒ2F,
¿?&óoŽ?ƒ2F,
¼?ïøsôKË?H0ûÁ",?N0.ӈÕ%?H0ûÁ""3FGL J0216.6-1019@f"ž²gÇÀO闟ÄVÀ:.\|ÙÀ;â$¯â±;?åÁ&5ò@…¿1¯{@¡NÿÂmx¿Ý¦ë®±¦"¿ååënù\ù¿åå'Íò‰¿ïÿÇ|ÆAGNbcuPMN J0216-1017?ïþ-w°
?5õç†fbñ?-(Ž´ÿ,º?5õç†fbþ?ïÚØÞÞ?x8QVOó?rö"ù?x8QVOó?îyFIªõ?Eã§M´?¨kŸûePª?Eã§M´?î#ÄìHvm?˜¢u™g!`?­Ã±;x™:?˜¢u™g!a3FGL J0217.0-6635@r%/€UûµÀH1" [TºÀ9 vö¢½À;±ù‰Ä9€¿Ùß-#û@…TøØþ?ÿ®Ó_Ž¿á
WÍ,ª¿âµ‹ñ¿×ôöí1Ç"¿â_O_¨uïAGNbllRBS 0300?ïÿ«qM%?\×d®Ä?•#¬·/?\×d®k?ïò9\ž}Ò?gmp,*Ú?[FÃ[5?gmp,*Ø?ï×£kÝ]?woHÀÔÎ?t.JQv ?woHÀÔÕ?ïöúI©©C?JÿIîö0?Rl¬­{Á?JÿIîö73FGL J0217.1-0833@eÎWà&EåÀOB:`NqÀ:^XƒNÔyÀ;åú÷''ý?çNáAsì@
F`·{@£, šTU¿ß}Z"õ?Þ¿ãl³vS]¿ç‹MF¿éùWÿ½²JAGNfsrqPKS 0214-085?ëûŒÄi4?¿_--XË?ÀÌï'[0?¿_--XË?î,t&$.Ê?µ6Ëç³Å?­8½½v?µ6Ëç³Ä?éšØ
g¨Ó?²‡´'Ê@F?ɔŸÊa\µ?²‡´'Ê@F?á»qDYFl?·}4ñ/ï?܉wMs(?·}4ñ/ï3FGL J0217.2+0837@c"4 -œñÀHQö¬m²À8Ï}š_'7À;X}ÞR0N?җæEï£f@&âÙ(¦@ÍnB¿âSï¥X®\¿â›^HhW¿Ûx½­mc¿æáT~\|XAGNbllZS 0214+083?ïÿ§Õޝ"?Œ"C›?
ˆXš»?Œ"E»?ïòÚ4õŸŽ?f1ËöË	D?ZK–Àâ¨?f1ËöË	C?ïÍô–ø?~û#~'Ò!?y´óƒù?~û#~'Ò?ïýž·?-'À Ò¢?3
D߅y?-'À ÒŸ3FGL J0217.3+6209@`™ÀµgU?îÆ)ñkÀ8yÛVÓKlÀ:­´{/P@îcßxv@
Ç`|?üÌÄ>]ß?Ø%‡P8I¿çQk"ôÝÉ¿î݆þâHµ¿æËW?4¦ÙAGNbcuTXS 0213+619?‡¸üR5à—?""69ÙÓÚ?ï¡·(~?""69ÙÓÚ?*V>§/	o?K ²/_×?ïþZœ?K ²/_×?ÌVÎIx©º?µºÞò£W±?èêLm¡Õ'?µºÞò£W±?[–Zò~h?V4øðì<M?ïò4҆ÀÊ?V4øðì<M3FGL J0217.5+7349@`§Ÿì™ò@'ïÆ¡9¡À8šÞ>åÀ;_Ae%Ç?íxNµ¥@ì؏ù‡Á@BBàzS®¿çÉÍ#½R¿êv,g<$¿íNÀÉD">¿ïþ>F./
AGNfsrqS5 0212+73?ïû×ü%¶f?FèókÔ?@ i&l<?Fèókç?ì¹H¯?Ãé"»K?¿Â5¿ê†?Ãé"»K?î£ÔÊܱL?™m]ª÷9?¥Â³R4ë9?™m]ª÷>?äSyÌB'?½iCßÓòÎ?×Y
âgzü?½iCßÓòÎ3FGL J0217.8+0143@dE– hUTÀK5[ßú¦ûÀ7̄eTîoÀ;"‹›˜?ð­¬
µe¨@A*»?†©@‹ jC@¿Þ›Rú¬a¦¿ã¢
ã%§¿â˜rÉ\f¿åè×}æñÍAGNfsrqPKS 0215+015?ïÿ;¸Zo?萣"Ü?Xˆô²)%?萣"/?ïóíMŠá?cPjPÌ5?X%dêà@û?cPjPÌ6?ï6zE¸¯?'9ySkf?™0·HêÓ?'9ySkf?ïú¿ÿ´<?Cz4"óî?E/‡m?Cz4"óî3FGL J0218.1+4233@ap‰ßrïÀ1² Ñœ?À7Á¿ß~€9À;
~gäì@ˆĆØ@'Mp÷@ñ†‰qƒP¿ÞíC7À¿+¿ä_rÆ	ÿ¿æS=nj@¿ëöDyùã~PSRPSRPSR J0218+4232?cßÖxºãº?c¢QKԁZ?ïì )‡E?c¢QKԁZ?rQ°=?~Âì&+
?ïÛÝ]̞þ?~Âì&+
?­_¾óí™I?£©ËÑÉIq?î*Á&l?£©ËÑÉIr?a§_6'ý7?\_aª:?ïîX Én?\_aª:3FGL J0218.9+3642@a»»ÿŠ;À6ì¡`7x<À8Û§¦¢–˜À;Ccf×¥n?î3·#\m@‡¦ÞP­Â@› ¿ã…Ÿ cš&¿è…Ámüg¿æªÊo‹Q¿ïÿ؍ÚAGNbcuMG3 J021846+3641?ïìÂÍ)?i
›©
*u?cç=€2×*?i
›©
*t?ïÐÆúAt+?'Üa°Sm?wœ'ßEê›?'Üa°Sm?ï
Q &î?"pˆŒsj?žµÛû!û?"pˆŒsj?¿g'?~1ŠivJ,?Š'&:6?~1ŠivJ+3FGL J0219.0+2440@bbÇÿÞrÀAGñQçÀ:Oá4bÞÀ;ÀËÈÀΒ¿Úo3˜@^¸»F=?ý¶ô ü9w?ï¿J£!¿åo7ýr\¿Õ	äEöj'¿ÞšR=ÜÑÊAGNbcu87GB 021610.9+243205?ïÿ¬X5»s?òtCc?éò'#±U?òtCú?ïïrZ²©?iD3ÒÚ{ï?`û¥MW:?iD3ÒÚ{ð?ï¼ÿ
ÉËL?yº'®'Ž2?€À=M-4?yº'®'Ž3?ï÷Ô- A?HØ×`cÛb?PW¥¿}Ü©?HØ×`cÛ`3FGL J0220.1+6202c@`¤4_½Œ?î(ê@6b#À8ò=)HÏÀ:FÁÅ1ÍØ?ôܽîbž±@>jÉÍhÿ@\[ÿÛ¿ß¹¿³4¿æà± ÷[í¿æé  0ø¿ïû†ô{gOTHERspp0?x6@Qƍ?€¦—L›ñ"?ïϓ]Îs?€¦—L›ñ"?£Qê*bzÙ?¶h®*½?îÊá]YØR?¶h®*½'?ÂdÐ]צ¶?°Ž'—×?ëfËèŠR?°Ž'—×?¿+O"(Ú?°!˜Häs¾?ì–
zð?°!˜Häs¾3FGL J0221.1+3556@aÓjßqêÿÀ7{/à˜[¬À7œë"aq4À;
.óŠ§¿ìc²‡QB"@Š|p>@A(ƒÓà¿ã'›ê'ì'¿å¿aC*»Ú¿áùx¸‰°¿ã£ˆŒ<JAGNFSRQB0218+357?ïÿZ¬ð?ˆUb ±g?ªaýž¦?ˆUb ±ñ?ïèA$Úô@?sUÅnÚÖ?g¾Û%¿Õ?sUÅnÚÔ?ï˜Ã¬2–µ?ÁŸmQi?‰ÏóZRØ?ÁŸmQm?ïÿø¥Q÷v>Ù"ë©I†¿>Íj¸"*©d>Ù"ë©I}A3FGL J0222.1-1616@gÉ hUTÀP—L?ß À9|ÙGdCÀ;Ê+÷Տ?´Æ;'õÙ°@˜Hí¯›d@ÎñŸêìs¿ãìå5ú7ê¿èˆˆODa¿éënÆåµ°¿ß~ý<'h´AGNfsrqPKS 0219-164?ïþÉÿò,?$vß
@?#`Ý>·Â?$vß
€?ïóbŒÎ|Ò?c€W°ë'1?Y:æc]Ä?c€W°ë'5?ï¹`¤,{5?~P³þ‰?§Öôá2u?~P³þ"?ïÎånÜV?p±C¼}ô?xH'Ôüå?p±C¼}ô3FGL J0222.6+4301@a"Р+"À0ÄZ&–mÀ6]<¼HñÀ:
©yámn?ð‰•*6¢@$}õÏ$–?ýTÛ+µ:Š¿×>5фRÇ¿à¢L¢V£¿Üa|…Z¿ßCb¥ç…¶AGNBLL3C 66A?ï`3fz²?(`¼uÁ ?Œ'ó&aS£?(`¼uÁŸ?ïÖO\·?€"¢Á"?týX1Q¤a?€"¢Á"?íMn£!?§WO]¡6"?µ—ôŠæ÷å?§WO]¡6'?ïÿ"¤Ä\(?Ùì§îB?
ÖÎèõÍÇ?Ùì§î 3FGL J0222.9-1117@f @FA-ÀO¦ÄŸ×¡<À:h|°TÇÀ;Í8Ëùh6?"z)@…Ë[ˆ'?ý'ýŸþbœ?ïàMH欿ڝû'¿ã5Ÿ°E>¿Àa
ÂAGNbll1RXS J022314.6-111741?ïý3E"ù?G¼rÿŸ,?6eÖï8Ý?G¼rÿŸ
?ïò¦ˆE9ý?eëFÌÒ¿,?Z²ïuŒò?eëFÌÒ¿*?ïmæù—¨ò?‰iàç{"
?'C Í
á§?‰iàç{"?ïåõܚRï?cA:Ïöç?j
#e­°?cA:Ïöä3FGL J0223.3+6820@`hğס<@ãŸú[ÑÀ9¸À*'À;nºeÁû¸¿ûт"|ÿ@¼×ŒCp?þ£¿à€2ë¿èðÁFóµ¿Ø}j-4/v¿Ü¬è6ÆÌ¿¿ßšØŒ&GAGNbcuNVSS J022304+682154?ïýå ÇIÒ?)ô‰é'+?0Öùű~C?)ô‰é&î?ïÃß…4¥?'o\Ðñ?~x½e­ù?'o\Ðð?ïÈ°Ž|Dx?y«±Õ?{§¸ÁÝÄ4?y«±Õ?ïÿ¹â­Á ?ö+,j?‡T—ÑÃ?ö+,ä3FGL J0223.5+6313@`¢Í œÃ@ye`,¨À9 @ŽÉ\À:ãPl)?ø‹×D;@uÊ\…!?þöx¥-K"¿ÚAøW
æ¿æ0NÃÌ6ê¿êö‡uœ©¿ã"øSIQAGNbcuTXS 0219+628?½ÉKHE?Áçéhã_?ìFß–ù?Áçéhã_?˟‰T³ü?Ñ'eˆz?éªÓù?Ñ'eˆz?Ý¢Ñuƒéƒ?½©æõãS?á.—E>??½©æõãS?Ã|/F3e??´,=ºy?ë ô.s&¯?´,=ºy3FGL J0224.0+6235@`«¢_¦XÅ?ùáVèˆ?À9	"EœÂCÀ:lï­¢e?äc#c1}¦@tk0$µí@Íê€d?Øòtý¿çeg˜•›¿ëºÜ	€²¿âÑäÏ"£OTHERspp?âÒåtÎî³?ÐkTåÀë?ÚZ5b"š?ÐkTåÀë?åá^î5?Òh¿Ÿ¥?ÕÒä=B#˜?Òh¿Ÿ¥?Þ´—`ñŠ%?ÂT,æ‡y?ॴO‡:î?ÂT,æ‡x?çã…
ZGÌ?Á	Eo?Ð8õåKpi?Á	Eo3FGL J0224.1-7941@ržq_ˆü"ÀBAÉ¿Ò‡À:ÏO^À;ÎïS	'¿õuŽ²Š×4@-#""±Ö@ÔÏbpã¿égØt~_µ¿ßÊ1%€±Û¿Ú÷sË:Ñ¿ç‰Äl'6AGNbcuPMN J0223-7940?ïûy¸õ¡®?B}?Ñö?B)yA›?B}?Ò?ïì˜Ä(?ß?lh%âãÉË?cg;×À ã?lh%âãÉÌ?ÃÒó?‰U˜Ä{§$?yOCh?‰U˜Ä{§$?ïþj
p
?,«wC#?)_(ÿ_<"?,«wC"†3FGL J0225.2-2602@jéÂ?«ºÀQA×,uªÀ9C[m TÀ;ÚºÌH¦?㧦¤¼YÚ@‹úÇ1€@NÌÀb†2¿æoû
¿è™›fÅ©9¿è<Éøj¿ïÿµððÌAGNbcuPMN J0225-2603?ïÿ}Krƒg?QXâ{Tõ?V'¯"/t?QXâ{T?ïõ®µSA?`o´ò%?T¢•ÁY~Â?`o´ò'?練")¥K?Χs5(Ò?†Zwu–­Ä?Χs5(Ã?ïõ ™?OòAúWßÛ?U¾ÍÍéØ]?OòAúWßê3FGL J0226.3+0941@cŤ p¸ÐÀGKÏ`%ÆÀ9'y…ýÛcÀ; dYEìs?êÐæ‹Kx@Aw÷ˆb@}±ÿlc¿"£úhóŒ¿èFwÓÌu¿ÓE
MXDÝ¿ëjò›Ø'
AGNfsrqPMN J0226+0937?ïþ}(ŽéÄ?/C.´3±?(-wcÁ$?/C.´4?ïêÉ̾¼Ÿ?m•Quàn]?e63ACa"?m•QuànW?ís- ]Û»?¦²–?´f'ý"2?¦²–?ï€äý—?'}Mø_…?øFþšS?'}Mø_"ÿ3FGL J0226.5-4442@p_
߆ã´ÀP̀SÀ9ÙLvѵÀ;¶³ÑSDK?Ý~-Áü‡@É.²E?ÿF]7ãq¿âYËRE¿t¿è¯ÐôéeN¿´y´22hn¿ÛþÍýñªIAGNbcuRBS 0318?ïþxM‹Ð?1`]æ¼á=?/È{'Bù¢?1`]æ¼áA?ïòQÉ]«Í?d'ÍœÅÄ?[\mD¨g?d'ÍœÅÀ?ïÔÂ\?x¯yë}¦Ï?uþ}ñžÑ¿?x¯yë}¦Ì?ïÎǾ°?è?nk2ô[EÊ?xœ §àN?nk2ô[EÉ3FGL J0227.2+0201@d¢æàé´ÀJh˜Ÿž–YÀ9¦Ž.+ŒvÀ;¨è»?܏?ÐSkŒ–@	éôZ@VOàh
*¿äÂÖxênì¿ã¥ªbÙX¿Ì~ê­¥¿èîðL7AGNbllRX J0227.2+0201?ïÑw™Òt8?ƒ<8´+r_?wD3Åãÿ?ƒ<8´+r_?ïžLý»?'àê`[£?ˆ¬Àú?'àê`[¢?îÛµáüuÕ?œ±zÀ¶¿?¢D¡à8¢¾?œ±zÀ¶À?îsùôXK:?šq£Ù?¨À`º{Lz?šq£Ù3FGL J0228.0+2248@bɸ!ïÀAq[ßú¦ûÀ9´Á"tŸÀ;–[ßú¦û?ã›@§~ÎV@z¯Èe@öÿ /Å¿àÄø5û:¿Þ*ÀžýAñ¿àøº04s¿ìÌã6àVAGNbcuNVSS J022744+224834?ïÖ;*‡X?t‡å¦4¾?tâvê¼Sš?t‡å¦4¿?ïá™çæ?wD±Ä´L?nf€~‡?wD±Ä´M?ì\J'ß+?¦áo«¢âè?½«if¦?¦áo«¢âè?ï ¯ÿR"»?zDÁ©b'?‡Ô+wQ‰?zDÁ©b'3FGL J0228.3-5545@qc²?î,™ÀL<—à[õÊÀ9!Å;ÞÓ`À;Ë®4[Q_¿õcl´3Mà@÷°(§>@h)@@6ý¿â}KÌ ñÁ¿æ'
ÏfÛ¿äŒR•	x5¿éö¥8^@AGNfsrqPKS 0226-559?ïÿnB¥¦?¹â'+7ó?7«^‹<‰?¹â'+7Ž?ïôþ!Æ`Ô?aÜ.u%¶?V¼s>XB?aÜ.u%»?ï³53
^
?ƒµ¾:•ÈŠ?ƒ2³=h}Ä?ƒµ¾:•È‰?ïÿÿ æ>¦ljWôw#>žã?«ím>¦ljWôjP3FGL J0228.5+6703@`†‰_$RÆ@Ë# C+úÀ9‡½Q.ƽÀ;6O¥YÁ?½Š|lã@
òê|‹ó@ó° ™¨ˆ¿Ü@YM	"I¿ìP|V¿à*rހ¿¿ïÿ€m•AGNbcuGB6 J0229+6706?ï™ÃÍDal?Žï«b>ô?‰®ç¤Þ?Žï«b>ô?í¢{oëF¢?»¾øšfåg?²ì$€¥Êõ?»¾øšfåg?ë=(BNË?¨Îcsñl?Ã^÷îÄ×?¨Îcsñl?ìÃ?'ÿÜ?¬ûÁÊ´?¹æoP?¬ûÁÊ´3FGL J0228.7-3106@l«µŸôýmÀQ| À:Èá!§¼À<®ÎµY¿æ2¤[Ù3@d
‡ÃXZ@s`ù•¿ãóåVO ¿å'™³£c¥¿ÐZJÂN¢-¿Ý83<ZAGNbcuPMN J0228-3102?ïÿ'Ôڂb?‡âå))?JÉ_g´(?‡âå)Ï?ïó:3úP?gÓJƒ›(?Y‹™Úa`?gÓJƒ›)?ï^¼©TŽ(?'Å€Åñж?"(jÕn:à?'Å€Åñд?ï÷éþ_ïç?K.ÎkŽ6?P,@ 1Û?K.ÎkŽ03FGL J0229.3-3643@n~9ÀëíúÀP̖üõŠÀ9&D7guÀ;ËW`9%»?á¹ØRUÒ@½º@N@Oß_¡{:¿äpô(G³¿æ"þnIM–¿èÓŨôe¿ë¸V5õ8AGNfsrqPKS 0227-369?ïý¨ì3J?0·óŸäõ?2¸že¯®?0·óŸäî?ïóÀ_5ҏ?e©3Ü¥h?XA"Zã½?e©3Ü¥h?ï–ûÉcLY?"Š¥]i]?ŠA
§,é¶?"Š¥]iU?ïÿ-ÄÉO?Ý´Œ]-p?Gfßö0w?Ý´Œ],é3FGL J0230.6-5757@q…E€<ÑBÀKL®¿›‹âÀ:Ç1Ç"háÀ;í´£á8?à _ŒúÇ@¬²£UÚþ?úõ@|òÅ?ßîCÐuº¿äÝþùDп⏃0 ¯"¿æ5²%AGNbllPKS 0229-581?ïòJàr"Ü?^¬ýú˜©#?[j?ºD"?^¬ýú˜©+?ïìåø5,<?m2lgM
8?cÊÓÙ?m2lgM
7?îÝÿÝP?"…Ï?Šü_?¢ /Úþt?"…Ï?Šü_?ïAñuØ)?"ÌÓAMµË?—ÁÑDýzà?"ÌÓAMµË3FGL J0230.8+4032@aÓdÜY2À2€nÿ'÷À8ìÓXØjÀ;ž–"ì"?д>Ç¢'@z›Alo@e# ™5¿å©À‹Ôg©¿èqSlŽž"¿èé"¡¿ÝûžaTƒ»AGNfsrqB3 0227+403?ïü"Õ~¹?<µ,éÔ?;aWÄ
8?<µ,éÔ?ïÔ#@˜å·?"ÈnåòdP?uî_³$#?"ÈnåòdP?ï«©8
?€·˜f¼»ç?…>U±û¼l?€·˜f¼»ã?ïüÖË @q?4P$u¥?9I¦ýüoÓ?4P$u~3FGL J0232.8+2016@cýŸÓo~ÀBNº@NÀ:"7ÜæÀ;¦7¾³.–?áæ'²ƒ@)@Í$¶n@4ßxöâ¿Áô©Ú\ ¿èßiKaí¿æ¤ç¢Þ^¿¥g7"
`AGNbll1ES 0229+200?ï¸Üa@2¼?ƒöwvH~u?Èç¯óPÛ?ƒöwvH~u?ïéc-#xg?pÐä}W2?fœÒ܇—¦?pÐä}W1?í´ÈgŹá?§gÒæìÁ?²Y¼ÁÒ0í?§gÒæìÁ?ïHÛó?'
ªäT?(?–üāŸ¾?'
ªäT?'3FGL J0232.9+2606@b·žÀµgUÀ?n¢ ©XSÀ:Š°¬Ö)À;ÔîµTá?ݑwÿ‡o@.Ò¶p¿Ü@°ßŸã4ÿãë`FøÉ¿×Zp,>¿Ýc²£<ì¿ä§¿ zšŒAGNbcuB2 0230+25?ï÷0­sç£?Oßn±:R?Qž¥0»o?Oßn±:Qü?ïfîU…­¸?¤$™.ð…Œ?""5OJHì?¤$™.ð…Œ?ï|*À˜ÀŠ?‡á`¼?z§ìçîÊ?‡á`¼
?ìnÏú¯ð?¢ý‡þ¤"5?¼É€*€ƒ?¢ý‡þ¤"63FGL J0236.7-6136@q³SX"ÀI¦Ò?ÓT¦À8…´~êÂÀ;"Æü©3k?ç}¹ÝÂúw@äÇÉ@w:ßyø"¿àp°F%ˎ¿æ£ªGDk¿áހM¢A¿èˆ4X'AGNfsrqPKS 0235-618?ïÿ'2õuà?3mó@…å?sB¢‡áw?3mó@ƒä?ïô%šÔ	€?c›ãQ38?W´ÊWìýš?c›ãQ39?tõã?‡CÒ¼Ö۟?Ž¢Â‡´?‡CÒ¼Ö۟?ïÿü>ØM%>Ä·8!?V$>¾	=–ØY>Ä·8!?OV3FGL J0237.5-3603@n%ËßÒcÀPr¨æj-À9êøš°ðÎÀ;ªÞüz9'ÀëhnSp@®xù¼?ý»Ð@Ô¿Ôûè]ê¿ÚkNûï,ҿґ*2w¿âÞM[ä"yAGNbllRBS 0334?ïõñôÍ
?Tl[²¬è«?Tèeéµ?Tl[²¬è¤?ïöXäf6«?`ÞÞ Í?SN73'«&?`ÞÞ Í
?ï@ó)¡˜H?'|ӉVn?—ášËÌ÷(?'|ӉVn?ïÿöt$…>äWøTɇ>Óý¶øCI>äWøTɄ¾3FGL J0237.9+2848@b¯8¾øγÀ<…'ßBñÀ6ë7OËÀ:ûìƒKy@6?çÍ@ h(,ºž@*%³Bâÿ¿áêÀӚF¿æžºæÎß)¿æŒ*Š¿ê½ucÚEAGNFSRQ4C +28.07?ïÞNs	<'?qÜðÁäiU?pØÆ{aí)?qÜðÁäiX?ïç×^´k{?sB,qC?h(¡K""¨?sB,qC?í—öïË¿<?£â¿›×Oò?³@H¢/?£â¿›×Oò?ïÿ®9Y8?
/éD>^´?x±©²7'?
/éD>\3FGL J0238.3-3904@nþã€ßÀP0‹À'¢ÜÀ:uå"m/®À;÷©4AP,?×Í/@Ð溉©7?ÿ] D-¬?ï÷½À"-æ¿âÕ -qþ¿Ë\6;ÙÓ¿ç8€šR¸AGNbll1RXS J023800.5-390505?ïøz®>Æ?a0zäƒ$ý?NGçˆ:?a0zäƒ%?ïåFo·ùÓ?s>«€Øp
?j¹H-d?s>«€Øp
?ïÚ&é¾?"H‡…À›Ô?œd»"È=v?"H‡…À›Ò?ï]×¼"Н?E6¨~µ?"Em…ìF?E6¨~´3FGL J0238.4-3117@l¯¬ºËCÀP•‹B¹À9XõL»šÀ;hœøɪÙ?Íè»q@ñ@áü]‰ ?ý^%y¿ÒúÁ?ƒ2¿ã
ù;H^¿Ðá¢Y(1Å¿ÖwÑýÅ­AGNbll1RXS J023832.6-311658?ï÷šèŒð€?Pù_¼'Þ×?PÊ.æ2?Pù_¼'ÞÎ?ïñA]ï•_?fÁ ™Ã=f?]}D Õ@q?fÁ ™Ã=j?ïSÁ¯ìщ?ŠÍ"ˆ™M?•‡ÊeÏ?ŠÍ"ˆ™J?屢c' ?y7â.Ðl€?†<'wõ?y7â.Ðl€3FGL J0238.6+1636@c˜à¿]xÀCÏߦÄ%À74^¬]ÁÀ:¥žÜÏyO?÷³ÿEÅÝ@!M^|Y@…Öí¿Ý諍ën+¿ãÇoܘ&¿â6"׿æªÒîò3AGNBLLAO 0235+164?ïü½¡¨?7.â´¾º?:÷?ŠÃZ?7.â´¾¿?ïôkˆ¬J?c¯ÿe1Yø?W(Äî§nY?c¯ÿe1Yý?ï¦~kA?–5½¼?<Ë02˜?–5½¼?ïÿÿWôU¸>®Kϲþ>•uI	ŸÛ>®KϳXS3FGL J0240.5+6113@`õ¹pޏ?ñada(ŽêÀ5xþ'jöïÀ:%ÂÐʈO@K4[Ò9@]Ë5ó×Ô@N
Óî$¿Þ'Q¦»Á¿åt÷ù¡A.¿æÉÀµg¿ëS?bk…	OTHERHMBLS I+61 303?Ü-EÈÉUˆ?ѤA,&Ð}?áé]›U;?ѤA,&Ð}?¨æTÄ[?Á6.ga…"?î~AžÚ³º?Á6.ga…"?àvÆì"@ž?Ã/|¯ÝÊ?ßr&×~Å?Ã/|¯ÝÊ?µ‹x}Vwã?´FÍJR¦"?íNðU1?´FÍJR¦"3FGL J0241.3+6542@`½œÁæ°@Ñu @&âÀ9>$'ýÀ;9ݾŒ˜)¿ð Õugá@{«Ý>@£Gßg¯¿â:ê«@FR¿ãu.å4'q¿á}.\'[¿Ôb³ðC/¼AGNbcuTXS 0237+655?ïÐdß¾b'?uÑ8¶"4a?w͐ η?uÑ8¶"4b?ï¸iK«;%?'v©8p˜?å­16Ø?'v©8p˜?îW:DZëC?›µÈD"è5?ªŒ[ºQKÃ?›µÈD"è5?ïÜ\ԟð.?vÓ2Ãd?qѕ°è?vÓ2Ãf3FGL J0242.3+1059@d:¬ÿ§ëlÀE¬×5ÜÀ9£YË8À;–¥€éŸ?ñäŸANSö@Xéçå¬î@N_ƒô¿ãÔ—m[¿å³{œGb¯¿è¶8¤ißË¿ïÿò"5£ÀAGNfsrqOD 166?ïÝ÷35E?†~4¬½"?qfe]|}?†~4¬½#?îœbf?­¡¨_®S?¨?¿©ÙŸ?­¡¨_®S?ëŠ9'^÷v?®yúòÒ?Á׶"",?®yúòÓ?â÷]'¡ø?µk	"Š©p?ÚE°½È?µk	"Š©p3FGL J0242.7-0001@e"-@ªêûÀI÷˟¦#À9°}IúÒÀ;ɑ
ÙÝW¿å˜?	ˆÈo@
ΛzšOø@–€"û¿åsŸi½2ü¿äf>"z~¿åÿC!gÙ®¿×0T[¡çFOTHERsbgNGC 1068?ï¾ì°	ö?…žïB!\Þ?€DÓý»w?…žïB!\Þ?ïìÚLä?v	Öq8Ê0?c%쀳4?v	Öq8Ê/?îaqŠëO«?ŸÐu_Ñš?©èçQKN?ŸÐu_Ñ›?ïÚËÜ?n•šÏ>h?ròúršá?n•šÏ>g3FGL J0243.5+7119@`wL Õbž@$Ê· "À9h±Ä2ÊXÀ;r¨W¢~E?ڇKBƒ¶@}™èÉØ|@ãV€bc¿ÑÍ8[ÕØ~¿ä6Re¿âtÛ6ûrZ¿ã£üH‡Ð'AGNbllS5 0238+711?ïól¹0?]‰óZRá?YÛ'þ?]‰óZRà?ï'áIÌEž?™œ÷¯ ?G­Œî˜_?™œ÷¯?îÿn)¸yá?—°q0J"õ? 	dxaÞ?—°q0J"õ?îäÈw=	?Šð–†"âŸ?¡³xŒ/h#?Šð–†"âŸ3FGL J0244.4-8224@r©óà7ÝÀ@ßL߬£bÀ:tÇR9‰À;Ă´zÆp¿ø•€Túe@¤ççÛF@n­ŸàÛx¿ëÚåÇÎü¿áwëøÕþ¿ä8_öhZ:¿ïýÀÈÐÇAGNbcuPMN J0251-8226?ïÙ]6ˆþ{?x"µIÖS?sQd»€Â…?x"µIÖP?ïÜv)Ò?€à¥>ºõ0?qÄësõ˜?€à¥>ºõ0?í"qMÈ8?¢"Ö·ß?³\u'¾?k?¢"Ö·ß
?ïùƲKÈ?Lá÷^Æð_?Hå6Ðߦ?Lá÷^Æð63FGL J0244.8-5818@qf{à~íÀJ‰~¿ù³À:Õ¥¹cÀ;©ë-àãÛ?ғ&
ö4@
˞¤pb?û-í"Ti¿ç«/lìâ¿âˆÓƑv¿ÝE'"&?¬ùËÏ÷¥AGNbllRBS 0351?ïþ6"6?0'¶¶I?,Ÿ–¿L‡?0'¶¶'?ïóôDï"7?aªG	E¥h?Xv!»'¼?aªG	E¥k?ïÐú¡p?zVªßO¯,?wý¯Gôß?zVªßO¯8?ïïRõ?5³?ZbÆTØ?`­
ÀÊMã?ZbÆTâ3FGL J0245.4+2410@c7oŸËÀ?ȑ_8t¼À9)›«Â'
À;'ÇÖÃƔ?ðL"èÝy˜@JÃú@Mx@¦v pMp¿ä‡mÉqȿ稦&𯫿ꮇʅ¿ãä¼òAGNfsrqB2 0242+23?ïþcó/l?-dW:^å?)ÀÍ	?"/?-dW:_>?ïә˜µ¿Ì?¥pwg;t?v33¥ 9?¥pwg;s?ï>¯w6?"aÞmØØ?˜*K?"aÞmØÙ?î^~?œÂ\ªrˆ?ªH®@?œÂ\ªrˆ3FGL J0245.9-4651@p]_Œ¨ÀN
dàTiÀ7š¹y2ñÅÀ;F{jÚin?øeZ‡àß~@imãÞ6W@ÊA€h¿âißW=ÿj¿åðxô'˜¿è? Ÿ»OU¿éåb¶6;AGNfsrqPKS 0244-470?ïóq–ok:?V+eÝu¸?YÓ!)Š¬?V+eÝu±?ïóނëù(?bf¿6¹?XBú(
±'?bf¿6¹?î¶Ô–²~?˜æþá|y2?¤'¾¦"Ø?˜æþá|y4?ïðËÙûñ?_äkõˆE??^hLó¶?_äkõˆED3FGL J0248.5+4232@bÏÃøÀ.—VgÀ9û07EçÀ;Ö4O'åJ?ê¿7öûï@
'­õF=§@T̀K¿Ç¿éê7§ó5¿ØtKR¿êT™"·v5¿ïÿتrýPSRpsrPSR J0248+42?å¥þ"ï•n?Ëk@H?Ô´ö Õ$?Ëk@H?ÅûKoK~?˂eG¡Î?ê-$;­!?˂eG¡Í?çºêÒìC?³ †¦	ò´?Њ+ÔZ'{?³ †¦	ò´?Ë}qw	?³[aO"?é9 ¾£¢=?³[aO"3FGL J0248.5+6022@a¶â—?ç*‹_Ö:›À7рuÜ%/À:rgᐩ0?ÿXŽ¤ž@ÊÈ.›@Î`=Wyd¿ãââ%­W¿ä"Vÿ¸¿êµDøØnl¿ïÿšFçPSRPSRPSR J0248+6021?øØ[	D?Ç='fÕre?ëÉé=œ0?Ç='fÕre?MSƄ?`8b—Œ%?ïøœ+<N_?`8b—Œ%?Îw=Iœã?·!θT]³?èb0­˜Ç?·!θT]³?‰i2ýçãf?}øØÜùz?ïš[4`q?}øØÜùz3FGL J0249.1+8438@_qåÿ£¹®@6my€žQÀ:
ˆÊ>}À;鯣ÇÀ$"Œ"xs@Ҕ%'_@,u?È¿ßù7r÷³¿èÞ X7¿Ñô²_õDK¿ã&rèÕÁéAGNbcuNVSS J024948+843556?ïÿb¶¼Û?Ó0,ß	ò?¼I(dŒ?Ó0,ß
y?ïáé×=?y3Œ4‰?nèÿ(Âì?y3Œ4‹?ïÌ-$sã?z"èà–;?yéyíÆ>?z"èà–:?ïÿüÍ«ùH>ÆB­>#>¹' 5Á]>ÆB­>{3FGL J0250.6+1713@cí€í )ÀB‡dàTiÀ9î&'d@òÀ;Ÿ_ý–™?뿸Àâo@v`Y‡?ÿ½±žÉj¿ê77ÙO¿èM^»Ðù¿Â2MD¬Wa¿ÖÞº_3AAGNfsrqNVSS J025037+171209?ïû+9ŽÏ?AÊ1LØs?CQËÄÀW?AÊ1L؂?ïà'"'5¾?yŒªø&ä?onl}ÊAA?yŒªø&ä?ï1ˆ¦ÆÃh?' $bcE?™Îë'''×?' $bcE?îï²Ü§°K?•dî@#,Ö?¡Ò5"ûZ?•dî@#,Ö3FGL J0250.6+5630@a[¦?šIÃÀþ¬@:WÀÀ9ŒEÅ.îÀ;FÙõª;¨À{èP¶Ñ¹@z<Cþ¬?ÿØրÂ-¿Þ\†öÅ¿èVF3HµY¿Í›Ý '¡¿ÝEX"ƒÅAGNbcuNVSS J025047+562935?ïùm·ÅT?HꤴÊ2?JHõ êµR?HꤴÊC?ï 4¦3ÇG?´r*MÆ_ô?›ùk9‡?´r*MÆ_ô?ïX7ôX¥?‰'òŽ0¾Ž?ùtë~?‰'òŽ0¾?ïÿù·Ÿ‰>âÝ©ŒÕh>É!ƒÚ«ê>âÝ©ŒÙ3FGL J0251.1+2603@c=X@žUÁÀ=ƒ?ÀàÀ9´üÄâÀ;£XãÆäU?ó³	ªx¹û@Ä;dÚö@J3q¿Ôö¥»][¿ÞAç«ö=‰¿ç{"SÈeE¿ïÿƒ€¨†òPSRpsrPSR J0251+26?¾ö˛Ѕø?Âߒݵ+ú?ì!&Œ…ïA?Âߒݵ+ú?&ú	g‰?§àõÐÉ¿Ã?ïÈ/_´Â?§àõÐÉ¿Ã?Ë Dɱþ?±LD5—?éî;€?±LD5˜?¢N{oþʑ?‹ø9…C=?îÛIW?‹ø9…C=3FGL J0251.5-5959@qu€?öÀI¤¨à^z	À:phŠ'¿À<FJg,_?Í퉊¼
@еd¦GÓ@QÇߨ½¿É2Å&\­w¿äÍÎZýÆ¿áåǥϦ¿ïÿ¤D1LAGNfsrqPKS 0250-602?ï¾·"©ƒŠ?š}!ƒº?€R՟[?š}!ƒ»?ïz(ŠóÓ=?–	¥ƒ3žI?ºî¡…˜U?–	¥ƒ3žI?ëLMõù·?¯"=¹D"?ÂÎː((?¯"=¹D"?íÐw5ž? Ñ¹—Y«?±|FSP? Ñ¹—Y«3FGL J0252.3+3830@boaŸÂ¨‡À2ˆw"^À:[àíìEÀ;Ò¡áf·Å¿ðvĖrs@'¶YÃÀµ@ø-Ÿ nË¿ä'†#+d¿ë¦Æƒ»š¿æ¡«;W™ð¿Ð–Æ\˜AGNfsrqB2 0249+38?ïþ'ÏsÀÝ?/óS£ºö?'ÓÃò12?/óS£º©?ïÞ"ÓYÈ?|ñl§'•?pî–Sr´?|ñl§''?dŸð?"`k>'h?ŽæØú&?"`k>'h?ïþ²þ4E|?#z[õç?$л¨6~?#z[õæÒ3FGL J0252.8-2218@j7ÿyÈCÀOŸÿå(
À7–>Õþ¤¶À;"™.9Ï?ø¨y @Ò'{™ÿE@ª"—(ü¿àÃý1…g¿ä£·F4m¿æà*R—… ¿çcò:<AGNfsrqPKS 0250-225?ï÷«{L"?QbÏQg»?P©	füئ?QbÏQg¼?ïóø!vïÒ?g£þ9y?X½ `?g£þ9y?î‰zŸi/?›ËÝ8M?§hV	n,þ?›ËÝ8M?ïÿl(tô?"RËQ»ìs?zñaI?"RËQ»ìQ3FGL J0253.0-0125@fMþûôÀI'/`?Û¸À:Q¢xåÅÀ;ÄüÓ$Õ¢?ñŠ´(æþý@=s˜Óöã?ÿ.Î*L…?ïìóǞ Ñ¿"ÙsÌ+Š¿áê
ü™T¿æÅ&TŸáÕAGNbllFBQS J0253-0124?íŠQ ü?¶dNŽß³?³¯íwø?¶dNŽß³~?ãƒà‡ì?Ñnñ;¦ÌÓ?Øø>ñØ'ä?Ñnñ;¦ÌÔ?å¶5÷‹²!?¸Ã锨2?ԓ"蛽?¸Ã锨3?Ðå~±wÂ?¸IÓò~­?ç@§|Ä?¸IÓò~­3FGL J0253.1-5438@q— /µÐÀKVK`P¢°À:iONóÀ<
Ñ@±¡¿Ëùî8W_b@½'ÐÄÿ@"°ŸðuÉ¿âps9ÕÜ¿æHŒ'0Tî¿æ"×½cÍ¿ìUaÀS0˜AGNfsrqPKS 0252-549?ïý@ue‡??GÅ´¯$×?5üT×Ó¾G??GÅ´¯$³?ïóÞN#ô&?d<s´É¼é?XCc¸µ#?d<s´É¼ê?ï°<‰û5²?'0w(a*?ƒð݁2"`?'0w(a*?ïô''õm?Q)ÞíŸÿ?W°Ýô"º?Q)Þí 3FGL J0253.5+3216@bÞ>ߤ?æÀ7๿©Î›À9±€•Ó;À;*,ú4¿ø4w
þp@áܼ.@k@?
W¿å,¶Á6…g¿â
2Ì
¾¿äï«õøÑI¿"ÁjÕsAGNbcuMG3 J025334+3217?ïÿzmj8Ÿ?žKyvö?²R¸ìÕ?žKyw—?ïçÂO§î?wÉÚ
R[Z?h=°þXI?wÉÚ
R[Z?ï¸	®ž?ó?¬›'?ü}»TX¡?ó?¬›'?ïÿÿ£ÊÜ>b 䍊M>‡
Húâ³>b äŽj3FGL J0253.8+5104@a¸ ٔ[ÀcßÎ\DÀ8´w⏬±À;7ÞUõÖ?ÛJg@C˟¦#@Z9€ª4q¿çEZB¡¿ç¥¼'—ó¿ç^†7Ó¿æÎæ‡ÞÜAGNfsrqNVSS J025357+510256?ï÷Ô£ƒ9?NšQ˜kï?PWæ¸ùŽ
?NšQ˜kí?î{ÕÓ±e?±´; Á?¨B¯BÄéª?±´; Á?ïlË·­…˜?‹ðC$ü?'f‰
OM?‹ðC$ÿ?îß¡]{¨?'
Y
E£$?¢ê(Nµ?'
Y
E£%3FGL J0255.8+0532@eFð¸,,ÀFÌëÿ—û4À:L‰°îIõÀ;£´©^3?Ñ¿tâ!•@
€Ý°ŸÅƒ@Ž¹?|AÅ¿Úkk9É¿äÁw:ß@¿Úo/@h¿æ÷–<ËkAGNbcuPMN J0255+0533?ïýb
²r?3#Ÿâ,x2?4ïg'lfC?3#Ÿâ,xL?ïçNk'?n!°*³É?h±åå"mÞ?n!°*³É?ï\Ô=Wn?–4x›Å?"exU@?–4x›Â?îÿƒÄw)?ŒÓҁš? 7ød?ŒÓҁ˜3FGL J0256.3+0335@e‡y¿ß~€ÀG{íÊ»{À:;ëß·‹À;©ãiÇC÷¿÷YeqžÓÀ@
|=&|?þVE^®â¿ÙÉ÷9 Ìÿå€øiø[
¿ßaœ;¤4¿Û%¸«6AGNbcuPKS B0253+033?ïü^ç°ýÃ?:¢büMy?=Âxí¹?:¢büMY?ïòùv¨±?dwqöêó?Z
®íJ?dwqöêô?ï[Œñª^?Œ³8˜Ï€?"ŽaÊ´>6?Œ³8˜Ï'?ïþy†º*½?,<Ãêþ‹?(g"]TB€?,<Ãêþµ3FGL J0257.8-1216@hsÿ¬*ÀLr 6×-À:¶'Τ=À;ߎ¿K
?ßғ»‰-'@WðK'	…@Òýßê5é¿Þfé=¿ç;æqÓEÒ¿è\+´d1¿è71¹¥A‡AGNfsrqPMN J0257-1211?ïþg`±[Ô?0›­¾5d?)‰ôêBµ¯?0›­¾5?ïó;¿wÀ?d
ÿ1fÙ¤?YˆÀA?d
ÿ1fÙ©?îҔíü¹'?–ý<¡^öü?¢Ö± 4fÒ?–ý<¡^öÿ?ïÙ\hˆû?eö@¸xRY?sQË»þ'x?eö@¸xRO3FGL J0258.0+2030@cßdÀßXÁÀ@¬‹ŸÛÒúÀ9úá:B.À;{E	õLH¿õq.÷iÐ@'Ý/p…ú@!VÇE¤¿î[r:"U?Û¶æˆñ½¿ä]}«ô²¿Í.–Ì	ÙHAGNbllMG3 J025805+2029?ïü=&‰b?CŠ™]?>Ë·œïk?CŠ™W?ïíçó¨¬Ø?ow/QmB?bWS(?ow/QmA?拓Çh]?'µ<ÜͬÇ?…ßN%è¹7?'µ<ÜͬÂ?ïÿ!|H™"?Êÿœä?ÐvìÍqè?Êÿœe3FGL J0259.5+0746@e$»%_5ÀE§ÒàD²À9E<æÀ"À;qkI$6@?ÙzAµ,>@ÇâöYã÷@²v BÀš¿â9˜/¿¾Ð¿å?U÷i¿ßK|‹ýàÒ¿ìfçsI×AGNfsrqPKS 0256+075?ïû
+Êù?D³¶‡ª?C×Pԁ?D³¶‡?ïñהYÜÆ?g]_ÆRK?\P×LFvB?g]_ÆRG?î±ëHòÛ¢?ž'àŽÔ¼a?¤áKpÒEå?ž'àŽÔ¼_?ïð8<©?'?SÎõ<Gô?_†­±V?SÎõ<GÞ3FGL J0301.4-1652@i~à°¯`ÀM"€ŸÍAÀ:Yx°"À;ßÿê0Šâ?îöŠâáP@*³In@4`BŠê?îÊ«ÖÊ+¿â²W¿Úv¿ä¼G_°¿è$å?èÖÌAGNbcuPMN J0301-1652?ïŽVÑHo?'4loðg?ŒjK­ýäD?'4loðg?ïÉ
@¶?"(É{€Î?{z¸@_¥?"(É{€Î?ëhǀ`ìV?¯Ø?êu­—?Â\áþ|N¨?¯Ø?êu­˜?ëcT¡øN)?¯ÒÂÈ?Âr­xÇ]?¯ÒÂÈ3FGL J0301.8-7157@r ÿâ£ÏÀDߏÿ¼ä!À9©&Á½¥À;ìAVâdå¿ýÛZY<Ý+@ѾÎ\nì@ -à
q¿æþ¶"Ç¿ê¿çd…'*W¿é9ð¸Jšê¿ïþ×;ï"AGNbcuPKS 0301-721?ïÿ¶_sÑ?ƒ™M$?h£¿Ö?ƒ™Me?ïòJ"_?h4]"Ä?[j÷Õ@ú?h4]"Ä?ïÙóHêÞ?q'kQž?s[Šö¥?q'kQž?ïÿÃݓJº?à§ó|N>þ6Z¢OØ?à§ó|3FGL J0301.8-2721@k =ÀTïFÀN‹_ !¸À:ÃhÍJ¡À<îл?Í°¶h)@
`+¾ß@CA¿½ð'?ßóä²áX¿Õ¡ Á"–û¿çšS|:p¿ãºØ0AGNbcuNVSS J030158-272754?ïQÅ9*¢³? " ¡¹Z?•ÇXÚ«©'? " ¡¹[?ïå¿¿ªw?¬*¥Á.û?œH
±V?¬*¥Á.û?ì½ɺ†·?ªpRWÝП?ºa²+Ê>?ªpRWÝР?éÒW½½?´âL'?È·£ž¡	?´âL'3FGL J0302.0+5335@aµt!-wÀÎëÿÂîRÀ9±ôafLÀ;RN©±>Ò¿ÕáVՂ[˜@­Sk7¦@'€L–‡¿Ó^(²Ú:ý¿çl*³e{¿ê½·õ¾ø¿Ö—I³'_@AGNbcuGB6 J0302+5331?ïÛµ"ùôs?sZ{~¸ ?r%nƒÅö?sZ{~¸$?ï2ƒNEš?¬íOyuM?™¯–7\lÒ?¬íOyuL?î
OMõªÓ? ùÙâLÅ?¯[ ¥RÉ? ùÙâLÅ?ïìaJX4?^Hˆ¨:È?cžñµ§ÊW?^Hˆ¨:È3FGL J0302.5-7915@r|>KZÀAýVÿÁßÀ9æêºô]À;¾˜Ã°ÄYÀÆã<û³ë@:Æ¥k_@R_žK/¿âß
e²ü¿è†BPÿÄ=¿Ùv?/Y¤¿ëæŠx
õõAGNfsrqPMN J0303-7914?ïÿÔbåkR>ò,©kJ~š>õ΍JWKú>ò,©kJy¿?ïïfÑúå#?lD™´'dœ?`™.ݐ?lD™´'dš?ïßGˆþ<?t×°2aØá?p\@;€â¹?t×°2aØà?ïÿùNwÙ>ÚoÝS8îé>ÊÆ#̙–>ÚoÝS8ó`3FGL J0303.0+3150@c"CŸý`éÀ79՟Ú%{À:1æÒ1œÀ;ª²²oSu?ét4'®ÃÍ@
š{'pÖ,@…¿rÇ¿Ú¹éï¿åsÍl¯Ö¿Ù¾Uà *‡¿ïÿÜBê}AGNbcuB2 0259+31?ìéºfH$·?ÃZŸl¯&?¸²,;ÚJ?ÃZŸl¯&?ä-Ö±ÙÂ?Ðxn®ã«?פRœMÚ}?Ðxn®ã«?æÑ5SÃÚ¢?º—K--0í?Ò]•XxJ¼?º—K--0í?áҋ:?À¹ ô%«?ÜZéˋïý?À¹ ô%«3FGL J0303.4-2407@jÔ5 ÝDÀN‹`òËÀ7qJ½"sæÀ:¥C'&Ò¿ÏÓXî@ÞõCc'?þ±Zá"Z¿Ø,ôˆ¿àÉÇ{C)¿Üs,aK¹¿Ým8<²béAGNBLLPKS 0301-243?ïÿjÎ#dï?Èü­EQ?¦;"bP¢?Èü­E³?ïö	.ê‡9?`SATö`?Sí¢*ñŽŸ?`SATöe?ïÏ£sá»°?€Mh½>6?x.F"'§?€Mh½>8?ïÿþl럻>¶G•R:>©1Fcã>¶G•GÔ3FGL J0303.6+4716@b ŸDÔEÀ#¶î#;nÀ8SJM++þÀ;N"šVWû?çÂ6oÂts@å-oÏƧ@D¦€1釿㞎ŸÚ?@¿ä¯àWæh¿äú"â?¿ããœl²°ÂAGNbll4C +47.08?ïüª[aU?9@µ:á£?:­#"õS^?9@µ:á½?ïT–_ò²q?¡±÷Հv?•m4©±Ø?¡±÷Հv?ï˜'6Ny?"QàA³?œlû60Ü?"QàA³?ïòàÖB?RßÔyja?Z?õüS{p?RßÔyjl3FGL J0303.7-6211@qƒÄßÎ1QÀHZ$™ù;À9!ý¥²¬À;´Ñ¤¢â?絶"ï̵@ëxˆ§Ú@®ZÀr¿ä8ÚSÀhÞ¿çVbÔ¥M¿åD'â7†¿ê€?(ðö3AGNfsrqPKS 0302-623?ïúìý!­÷?FX)\Ža²?DLyH(?FX)\Ža¬?ïßî#—5?v\d ¸ß{?pî4~e‰?v\d ¸ßy?ºçÔ%?…ŸÅ Æ"é?ŽÜ'F
öã?…ŸÅ Æ"ï?î©ð­a† ?"Œ…âé¬ü?¥`õ)çž"?"Œ…âé¬ü3FGL J0304.3-2836@kõ¤€èȬÀNWþKZÀ:òº.d—YÀ;æÃ$º?ðíÇ¢@gËOKE?ù½AÑ6>¿ï»¹/7Å¿Ý㔏nm?톣Ùʝ¿ß…±">jAGNbllRBS 0385?ïâZà"
?rð¶‰!"?m¥ãlö@?rð¶‰!#?ïåÅ(-Ü?9,­Ðµ‹?j:ú×Ò"ë?9,­ÐµŠ?íȐB;Ó?¢\z…9fS?±»íî!g?¢\z…9fS?ïq)KÍ?®å×\G'<?'Ú֝F_?®å×\G'<3FGL J0304.9+6817@`Ù´ßݵ@!*ŸæºµÀ8±ÕORM«À;PgžtÊ­¿àiÐu›/@‰7jöC@Á`)áP¿é]£G©s¿ç5¬âC#
¿éÞ6%DÌÒ¿ãQj͘ AGNbcuTXS 0259+681?ïç/#³¸ñ?h\)р?hÐÜLGÁ?h\)р"?ïI@·@±K?§ê•0ÿÛL?–×ééÖ¤?§ê•0ÿÛM?îP}‹9š?B'to¡?ªø'Lf&e?B'to¤?ï=$Éõ7?‡!Ìê~Ä?Œ0¶Í'²j?‡!Ìê~Ä3FGL J0305.2-1607@i
l <K
ÀL'BàO`À:Š:¶µ3SÀ;Æjd!èˆ?ç·Uðêc@
x¯¸k?û!Û­?ïºSzÍR¿éévÉ¿º6'äÌ¿»Téj¬
#AGNbcuPKS 0302-16?ïþà¢?)dëè4{?!ÿ"Õßì|?)dëè4Ù?ïò†j€?f$`šÄ?ZóûÑ+%?f$`šÉ?ïg½½¸¬]?Šç3'ò?"HHêtY?Šç3'í?ïÎÏ秗²?rŒqB•q?x˜,4'/?rŒqB•l3FGL J0308.0+7442@`w¿Â"O@,o[Ao6À8ó¸ÒDÀ;Ý@ï´Xb@H² y@\z-m¡n?èh°n$ÿF?ã±i¸"A¿Ò:…ÚAvå¿ç[ooyŠ…¿ïÿñ­µcPSRPSRPSR J0307+7443?x"¿s$±?ƒ'a}{?ïϺ¶ ?ƒ'a}{
?g†CAˊ?vHf7fôK?ïèy¼ê¾4?vHf7fôK?¯"[´8?¤€èÏ£?îÊD¾}?¤€èÏ£?HÕòÇ)J?CÞ6v¹€?ïùʃ\6?CÞ6v¹€3FGL J0308.6+0408@eÜ:Ã.¾ÀF;à0VàÀ9¾Î?""ÆÀ;#†Ö?ÛÏÐÄsq@ðE®_ú@'‹ßǦG?ïðBÐ+ž¿ê,²€=¿Ì¦†iр¿â¢æ1ð
AGNrdgNGC 1218?ïÿ¥}¶Ý?	fE[I)?– 'H¥×?	fE[I)9?ïê×;k
[?n_"#æ­R?e(Ĕõ¤"?n_"#æ­W?ï¸îuÄyº?}œÐ<?ÄbŽá'P?}œÐ<?:±¤o?€bwúˆ?WqS–ä?€bwú‰3FGL J0309.0+1029@e%F?ÀCێÀ!ßÀ8kÖÛCˆÀ;-T®­ýÕ?öÝ7ì*‹@™»þHp?ÿã»(Š¸¿à.–PŽã³¿â]ÎUŸ*¿æžƒ8â¨4¿ä
(|Bh'AGNfsrqPKS 0306+102?ïúb—Ÿ¿j?NCËi´?y?Fu¡T·?NCËi´?t?ïñÓåÝ[ù?fIV¨¤ê?\X4EH¾?fIV¨¤ø?îiÞ&¶*È?¦ñ¨ƒ÷þ?©b"S{?¦ñ¨ƒ÷ÿ?ïþ,cž½"?.¬þSzcÑ?-9Æ'¶"?.¬þSzcá3FGL J0309.5-0749@gš·?1n7ÀJWÿ›V2À:åsŒ¿—À;¬Æ8^_?Ϥ'౟ä@Lªhö‹?þöý?†RÀ¿Õ}¥kΞù¿âéC¡¦"?µá݈ºVÜ¿èœ)×È\AGNbllNVSS J030943-074427?ïäÕ¬ uß?x"J-±"?k*S_Š ½?x"J-±?ïéÞËðR?nûrô¡'7?f!4ã®.?nûrô¡'7?Ä~™?aB®}-?¦føgû?aB®}-?ï²<™3³?yїѺ~?ƒpý³h?yїѺ3FGL J0309.9-6057@qa¦`ɊÀHyðßьOÀ8Ÿ' <¶À;¸éÀùZ?èªXðeÞ@׌yËs@_žŸ½Êü¿â!©¢?h¿çÚñA
¿ä;Ýòö}¿èb]{AGNfsrqPKS 0308-611?ïÿ,mÓj? +â:Gûc?:rE'ðä? +â:Gû:?ïñ»ï Ñ!?iw÷ØñP?\ˆ ¾]½*?iw÷ØñU?ïƒÞS4+é?ˆÛoý£?k2õÞ?ˆÛoý ?ïìùqýâF?[¯O›¢?cŽºD?[¯O›¥3FGL J0310.4-5015@py'ß֔ÍÀKr<à[À:3maÚÀ;»€šŸS?ìêjûݗ±@õ;Øbç?üÈ>Ï¿éFчƒ?Ö[4®³\¿ÒÑe™žy¿Ö|뗬ô.AGNbcu1RXS J031036.0-501615?ïÿ\zÆîU?º"êÒ[d?p§"5oÓ?º"êÒZ²?ïîT¶=?u?l–ƒHà?a«IÂÀŒ+?l–ƒHà?ïc-Ë9q3?'f¢0¹.›?"šF˜Ñُ?'f¢0¹.š?ﺡšº4F?töQzº/G?W™Qrîµ?töQzº/A3FGL J0310.8+3814@bÝF€"À0ñà18‡À9›á·?œÎÀ;š­•Ïà~¿ø´Ô2œµ@cÏÞ$8@c x›r¿èÖÚJlh¿èBxŸñCò¿ÖŽ*ľz=¿ékë-ŠýŸAGNfsrqB3 0307+380?ïÿÈkÎ>L>þ~à"ÄIm>ûÊàÙí~>þ~à"ÄIr?ïÛ⡽ø?€ÇdëRUª?rö¯!ê?€ÇdëRU«?ïÈo¸]P?€Vu¢$%?{Èr#ÑX¿?€Vu¢$%|?ïÿì6œ>çÙòHƒ40>ãñoÉd:ü>çÙòHƒ*ò3FGL J0312.7+0133@fP†þ÷ÂDÀFÁÿÑÀ9$5Ý1žÞÀ;×xø?ÒSDܺ@'èá'*@B¦@#¿áëŸè,œ¿ä
ÔÝp¿ãÁ&~¢zò¿ãÓgTmãAGNfsrqPKS 0310+013?ïÿ+ÜX`,? Rr©S\‰?"tóúhÙ? Rr©S]?ïô—ÿ-½?cʝiû,?WÒФƒS?cʝiû0?ï¢%c<tú?†f-"˜?‡v§0âÁM?†f-"–?ïþŸuFtñ? ¤+cü¬?&«˜±	×? ¤+cüà3FGL J0312.7+3613@ce`A‰7À2mêÀӚFÀ9ö"ö¥
kÀ;œ'«hÎö¿¡](þlR@Pà$ÃXÛ@E"…á׿ä'
Õ#»ú¿åàÆ£V˃¿âÑz­Ž!¿ãRt‡ï×AGNbllV Zw 326?ïþ•º™ù?)£¯ëqÓ?&¤V`ntn?)£¯ëqÿ?ïŀÚóæ\?ˆxë¯}äL?}?'†ÒA?ˆxë¯}äL?ïÍæjp9?xJÔŸk"?yýÊÇãs?xJÔŸkŠ?ïË@̵Ù?ll½·uÁ?z_™¥qß?ll½·uÂ3FGL J0314.3-5103@p…B 6mÀJýJ 7BŒÀ9˜0P)ãÿÀ;ÝÕC"Ó‡?Û«Qß¾
@oŒhC5@3üu¼¿æô ¦ò%U¿ãžlO'ì¿æKr7#¿Ù©©1£LAGNbllPMN J0314-5104?ïÛ}‰g	?u~:ªu†'?rA;|Lz}?u~:ªu†?ïâ&ê–`?xu§XÝíÃ?mÙiŸbá?xu§XÝíÁ?îYhç)›‰?¡ Ä('n?ªiqfGs?¡ Ä('o?îd4&›Ü?Ÿ#~ÏIÊv?©¼½Ÿ¦BH?Ÿ#~ÏIÊv3FGL J0315.5-1026@h7¹ÀëíúÀJ=Ÿ¿™À:@¬˜yßÀ;¸­7Ü`À«Ðo¼@ÔÓêÎ?"@GÑ?Î!6¿æfݲMD¬¿æ™¡Ž|ýN¿×"U0¤¿ê™ñùWlAGNfsrqPKS 0313-107?ïÿðe·«	>à&Û/¾$!>ß4©í«">à&Û/¾'U?ïõJ÷"[Ê?cŠ]@Ÿ€\?Uj»HlV?cŠ]@Ÿ€^?ï܅*TDµ?uߊޅu?q½jÕÝ¥e?uߊޅz?ïÿý¾Ømó>º#§‡ÿÖo>²	<mÉÞ>º#§‡ÿê3FGL J0316.1+0904@eƒ  ôØÀCÌ¥ 8LÀ8aCRe'¢À:õÍêÙþ?áØZx2
@°¡€mΐ?þ©; jM?ßÄèÅÚGè¿âÖ¶ÓÕÞ¿ÜR­Ÿ¾`¿×ïNBßAGNbllGB6 J0316+0904?ïþ›µNÒ ?(Dù"ÈSˆ?&D«ÕõO?(Dù"ÈS½?ïìibûh?j-A?c–ø˜í?j-A?ï¤Kˆ¡€?†Ú#jž?†í8Ý× )?†Ú#jž?M;ó?zÒ¢J¸•Ÿ?‰,±9ƒ?zÒ¢J¸•›3FGL J0316.1-2611@ku‹y¢ƒÀLá@&`½À9™šMÀÀ;Ší~óûæ?¿^&"¸@'k£<"?ýµu_Óz;¿æ4©: >¿ÔS"™Tq¿¿ÓLw¿vš^¿æüv.õ$ÉAGNbllRBS 0405?ïü*¶;žB?@n†/¹Î?>ªN#
ï'?@n†/¹Í?ïêš[Š
`?p3>_®ƒÃ?ee¤uõŸx?p3>_®ƒÃ?ï +š	( ?"ɬ¡6ޒ?‡õ}µø$?"ɬ¡6ގ?ïµñž°"?}';£''Ÿ?'ƒ˜S÷~Ê?}';£''¤3FGL J0316.2-6436@q˜Œ€AÀG` SÇþÀ9™m~ˆœÀ;Ƨ‰Fe?¿àáÕ#[W@)f],+@»ˆß¸ö¿æ¼ö‹ÝÕ¿äèåËæ¿Ømÿ!ˆ»Ñ¿Þ÷YñÁsAGNbllSUMSS J031614-643732?ïÿ»‹ >ý`è?úþI?7úú¯>ý`è?û?ïò+
â)?g^'ö©
?[éä;®}?g^'ö©
?ïà9LG5!?tŸ".j?oƳ¸ÊßÉ?tŸ".k?ïø'¯O÷Þ?D–,:ê—?MµBÀ "E?D–,:ê¯3FGL J0316.6+4119@bÅ}q?À+xÃß¾AÀ9š÷È3áÀ;1‡ëlm¿þ?0Õ4û4@
Acôq+'?þlËð¦¿æb;qE< ?ïéå}Ya¿âÂÝÌ4² ¿äTæ–nä1AGNrdgIC 310?ïé_­˜×?kÞ&æ0?f Rgó)ô?kÞ&æ)?ﮟ͍½?—:›na?"Xœ¿Ã?—:›na?ï
ØWóÍ?'BºÙf\»?ž¤þ5†V?'BºÙf\¸?ïü9Ѽèq?M¥_ák]ë?>1r¼)?M¥_ák]û3FGL J0318.7+2134@dZ{ 1ίÀ=¦B 6mÀ9CYLVÀ;FüÎX%¿ò%¶Ëƒ¡‹@ZaðàÓ??ýeŒ¿@)¿È†ÙI»h¿âÒÔ
³È¿ÚêYùN=®¿Å­åMn•+AGNbcuMG3 J031849+2135?ïÿÆ´>N©>ö}Ü⧲º>ü¥àجù>ö}Ü⧱ã?ïîú ôX×?hÿTú¨iŒ?a_§)´?hÿTú¨i'?ïØCbË.†?wl°,O:?sÞNšh¼^?wl°,O6?ïÿôôG>×ã¹Â
é>Öqöÿ‰|>×ã¹Â-3FGL J0319.8+4130@bґ"DžÀ*ƒ þ}IÀ6VdöúÀÀ:C,x.?úw°:ÅÏ@»ªõâoÌ?ÿŠ\º³¿Þza+OJ¿â%^>#Ò¿áXïYXz¯¿äĶ köAGNRDGNGC 1275?ï ϝŽ?Ôùmup?‡ùŒ¼\?Ôùmuo?ïÒñÈ ¹?‰Šd»Pé?~6‡?‰Šd»Pé?í!ÄH·"?¨%ü®#?·ÆñݺCä?¨%ü®$?ïèõú'J;?pâþVïЃ?g
nµÄ—?pâþVïЄ3FGL J0319.8+1847@d¢ß?–À?¬",2À9a6€Å=À;+£»[‹A¿ëq†œ€˜†@W¨ï¢æ?ù&:è¸?î¿^·ñH'?ÐG¢Ó¡t§¿Ñã%•L:¿È›ÀCì-AGNbllRBS 0413?ïÿŒJΫd?
â¡Äqþ?íLU'/?
â¡Äpƒ?ïðÊ}i"?j_؀»v?_æk,ø?j_؀»v?Ãè6?=.'{g?Œ]:…ò¿?=.'{i?ïÿ¹™¾ó©?¡ä<8r&?™C ?¡ä<8rB3FGL J0322.0+2335@dCsÿ¬*À;—ý_;ϺÀ9P»Ú6BÀ;F>{?æ°5­Úñ@$Š
ÛPH?ÿ"«€÷·1¿àtŽì'Â"¿àUšéоŸ¿ßçÃô*¿× cڒUAGNbllMG3 J032201+2336?ïö2×?Q'Ö&j¡?S›ÑÎQÙÛ?Q'Ö&j¢?ïßßÊ+2?uoÙ®hÆ?pêf·?uoÙ®hÊ?ïK•2ÒW<?•Fh)§«?–Y¥µ‰?•Fh)§ª?ïdzZ2ˆb?oËmI çt?|&Ræ»Ï¥?oËmI çr3FGL J0323.6-0109@fþßÞøH|ÀFœäÿÉy[À9tJLTliÀ;i'Q¦»Á¿Á7ð㓞ê@
¼¤ªnÓó?ý¡¾ Œ'u¿äv%7êI'¿Ú'e»4Ž¿ÑíÖ/ª›'¿ÐñèŠÃgôAGNbll1RXS J032342.6-011131?ïö;fñ‹?S³ò"(§	?S‰3Ìë??S³ò"(¦ü?ïðÄM_Ÿ#?fp•QŸ9?^we@Áº;?fp•QŸ6?ïf&wäÏT?Š)RÃ>?";1f¡?Š)RÃC?ïÞ·"£j?d]ôp?p¤n®xË
?d]ôp3FGL J0325.2+3410@czªŸ{ZêÀ2±Þ_œGÊÀ8ª_!ΆáÀ;r‰EŽŠ?öÖÒµ'@º³PÏÑ9@¤Íˆ´o¿åÖ2¼•Çþ¿ëÕf7I¿ëp§
ׅŸ¿å)y<¤AGNnlsy11H 0323+342?ïü•«…s?8/óÕà$?;R£Ôg¯Ô?8/óÕà&?ï…ûå%«?žóRñ9•?Ž;F¶•\?žóRñ9•?îíÍmÉk?–@…'N6–?¡#)/Ói\?–@…'N6–?é‹Y?£TÅé_™?®ö6agJ{?£TÅé_˜3FGL J0325.2-5634@pí ßÞøHÀHîà_PÈÀ9ø¦wÎm·À;øñ¼p^7¿ó¼lzQªÃ@í«B¹c@¹´ß›0ž¿ãu'ªMW2¿ÝÊÉTÊÚ¿åxþ(º^`¿àX ŽAGNbll1RXS J032521.8-563543?ïÐј¨Å?}¯9/¾Š¿?w—3þ+¼?}¯9/¾ŠÁ?ïïÕíV>?kÎû5è#?`*ë©Ã?kÎû5è#?î©Úƒðª?—ZÎdu–?¥bWÀþh?—ZÎdu–?ïõÀ>¼'~?SIÐ\»?T'†Ûi?SIÐ\¿3FGL J0325.5+2223@dub¯È°À<I¥ÒÀ8hpeÓÀ;Rs×Ûõ?õWéÞ«qˆ@BFBÚp#@¡êöÙe·¿ä¯ñuVKð¿é1-o#ú0¿èæ¨ãZû¿ïÿ?"éøñAGNfsrqTXS 0322+222?ïü—P?>P3€WÊ?;Cõ73?>P3€W²?ïÃFÈßË?‡Âºò¾)?~\ñ›ø?‡Âºò¾(?îÔà8ræ?—δQ׈.?¢±üxßј?—δQ׈.?ï"™¸XŸ?'r#=‹?›½ÌÈôì?'r#=Š3FGL J0325.6-1648@iÀÊ`ÀJy¢@1HwÀ8þ­-]À;.InÞÚì¿Ý4gX\@ØOØŽZ?üì¿[u?¼â¯ã ܿޙ`æÂ
οÚìýf?¿É÷7ô&óAGNbllRBS 0421?ïþr
3d'?'7W8Y¿?(ß,ɷܵ?'7W8Y¿j?ïóý¾¾\?dI"ãŽëß?X'ƒáF?dI"ãŽëä?ﺏ,á²t?€RƒéNÄ?\4Ǔcd?€RƒéNÄ?ïüKjøU§?6Ã¥øÍ+?=¤¨=RÂÞ?6Ã¥øÌë3FGL J0326.0-1842@iý^ß)ÀJÉ?Àà0À:P3:~À;ê'Ô©:!?̐õ_ß'@"KtG¥†@¤ìԍ¿ç­üÉÙl1¿ë¨ËÓJß?Îq€Ö()¿å)Rü{;AGNbcuPMN J0325-1843?ïÿ¨)ií?П1V ß?õŸ¥"×z?П1V¡?ïïqdÈ"?k\!gˆÒ,?`Ž›7Ýï&?k\!gˆÒ#?ï½1ür 1?|&'XÞê?€³€ãWóó?|&'XÞê™?ïçY%yzÉ?uÞÛ1Ñó?h¦Ú†…5¦?uÞÛ1Ñó	3FGL J0326.2+0225@f—ðŸ¥LUÀE7´_î}!À9^9£¼¡À;sK@p2˜¿Â2õö¼µ@Pß:šˆ?ÿøaՈ]¿å>êUÁ¿ß‹ß¼éá¿Ù¨ÀdDß¿áà¼:OÔAGNbll1H 0323+022?ïþ"ÿ"V?*"ñÝ?'íÐ
ڒ?*"ñå?ïðW,=?f³IMÚ?_QÙ§…Ñ"?f³IMÚ?ï²(h|ö?Õu¸ÒÐ+?ƒyµåàÂÉ?Õu¸ÒÐ-?ïã¾3߉ö?`FäfØ1—?lAÌ v	?`FäfØ1'3FGL J0331.3-6155@qO{`(^ÄÀG)´Ÿ¯]PÀ9¢ó_2•À;Ãþ+êi–?ßʆ˜ØJý@JêßÝK@œÁ€hp,¿Ûh€{¿áýý–æü¿ÙS	÷>0¿çè0ˤٔAGNbcuPMN J0331-6155?ïùæÛFK>?ICÔj"+ï?Hd'æÓî?ICÔj"+Ü?ïܦGvZ©?wFçJÚ÷?q¬ÜDÒ¬)?wFçJÚ÷?ï"B\Pá?—
ƒ1u~"?›·¼Tuãô?—
ƒ1u~'?ïA`ì¦ä?ˆå÷–ÍBY?×Óâk#p?ˆå÷–ÍBY3FGL J0332.0+6308@a~] Y§;@Ø4¤À9Aq
.W+À;E}ö¥ä+?ډWw`3Ç@
~ºÆ@¥àŸgŽÚ¿ä@Ë·€¿âbƒp'o¿çü5ïêÍØ¿áx¸É	É­AGNbcuGB6 J0331+6307?ﲧ׭Ná?Šs74®‡f?ƒV
¬GÛ?Šs74®‡i?Ev
?žÇcÎúÞ«?Ó`.¢||?žÇcÎúÞª?înòC°ø?•0?©ߋÄð‰?•0?îÌÍ.þa?K§s#:q?£3-Äï?K§s#:q3FGL J0333.4+7853@`Pz WŽ\@2{Ä¿¸TÀ9Ç~è=k›À;Ìëô°@¥¿à— ïèõf@%Ê>ýí@"Äÿ£ä¡¿Û•Dí'6›¿èñ%Ž¿Ôº˜ñí²d¿â_†«ßAGNbcuNVSS J033344+785027?ïÿ(ð'ý|?šs³ï¼?áï P³â?šs³ï†?ïÖOüªœ?|øúRè?tت±õh?|øúRè?ï¶$Œ ä0?€?7øÑ?'vÜ×Æó¼?€?7ø×?ïêë—OÁB?_5'HÀî\?eh°>½X?_5'HÀîQ3FGL J0333.4+4003@c3›Ÿ˜·À)óš?±Æ·À:ã'ñ·À;"b£cF÷?î…pƒ[û»@q¡Šÿ¢ã@æ¿ßÿY'?ïý°´,0Ï¿Ç$ۛ`‡ï¿çþÏ$¯¦¿ïÿ	ø&mAGNbcuB3 0330+399?ÎD­¥­	?Êq¸¤œÖ?ènԖ"¼~?Êq¸¤œÖ?ÁŒ¿€øîe?Ë__ffƒ‡?ëœÐÁÄf?Ë__ffƒ‡?ÛoººQ$E?¶ÆBDÍ)…?âH"¢×mÞ?¶ÆBDÍ)"?Í?3-Ђ?·ÍN¢®ñ^?è°34‹ß|?·ÍN¢®ñ^3FGL J0333.6+2916@dªKÀ5…šr¦çÀ8ÉðeXImÀ;=¨;i?ï-@ÓÃ6 #?ý¶É™"{¿ÏgÆ°_¿Ú¦¸f
{¿ÕNÇ,ò|¿Ú‹Ù"׬‹AGNbllTXS 0330+291?î½Ú¼#¿?¥©Oß( ?¤"T7íÃû?¥©Oß(Ÿ?ï6¥óÈÍÛ?¢ÓjÖeƒ?™+A†æDÊ?¢ÓjÖeƒ?íôñë$í?ŸbÙÈ=ݪ?°Xp¦Û€£?ŸbÙÈ=ݧ?êÝ2»jDß?¨È‡ô|ÿÅ?ċ5Vì‰?¨È‡ô|ÿÅ3FGL J0333.9+6538@aUDupÅ@p4 ½À9SFS¡hÀ;YÜ&Ü㛿ë…hßÜ@•ÒóW{?ÿ-! a¿ágZ™t
¿ã;©MZ•'¿ãEMVlj¯¿Ã3{}¸AGNbllTXS 0329+654?ïë‹ß;&?bqÏ;¥?dét ÄÙ÷?bqÏ;¨?ïȑ"ŽU?‰Ñ›'Hv?{·68ÿV?‰Ñ›'Hu?îëÛQã+?–µgSRj?¡BJáÍO?–µgSRj
?ïúY½¾¦?E'·"‡?F™	m÷?E'·"v3FGL J0334.2+3915@cG_ét£À+Æ 
aƒÀ:3æ/tbÀ; Öwpyæ¿ñ[µ
8h&@	'C¼˜L=@èØÞ\—¿ëž"('D¿áî‰~ª'¿Ñ§ˆUà˜¿â®+VÅßsAGNrdg4C +39.12?ïüæÌq6?BÃâvyz¡??ɜvXÿ?BÃâvyz©?ïb½,ȕ³?¤£˜RÐÊ	?"¨ZfíI«?¤£˜RÐÊ	?ãÞŸ?MJGÔù?‰_Gz˜b?MJGÔù
?ïÖ0º<?~.z'óZ-?tõg¢±b?~.z'óZ.3FGL J0334.3-4008@n˜ºà;>šÀK{Ÿ³À7ã$Õ¢^dÀ;ÁÀ)P[?÷	ÿºùf@
PIC•×@΁,æ=¿Ü¤SÃႿãoç‰ðõ¿ãT!šsx¿ä2Ó:éϬAGNbllPKS 0332-403?ïþqf澶?*îLò&+?(鑔ª¿?*îLò&+ƒ?ïñºˆ¨?gåÜåf#?\Šî¯éZ?gåÜåf+?ï8MÙÒH‰?'õ]ÞšŠ?˜öDŶîÈ?'õ]Þš?ïî½+ìl?_Ž³/w?aBÔÿ"_?_Ž³/w3FGL J0334.3-3726@n¶â—ÀK.Æ 
aƒÀ83A!…À;é/"Ê?òd>0<]Ô@@WŸÏÍ?ÿD@v½¢¿Ù?…¨Ö'¿ÞÐY©êt¨¿à
ƒsVS¿áÍróéAGNbllPMN J0334-3725?ïÿý-? b¢âŸ¼?}`NZCÅ? b¢âŸ#?ïê¯`†>\?mnWĆó¨?ePŸyÁ¤?mnWĆó ?ï"e)§?"îøA‡äw?›¼"ZßK
?"îøA‡äv?î®
ý›æ(?"¨‡dõ´?¥ &A†?"¨‡dõ´3FGL J0335.3-4459@o–``þG™ÀJs^ŸÈ‡ÄÀ9Èi*–¬À;ŸÈå·^¿ÿ€˜N?þô@ÅC–'¹?ýL ?µ?DkYÀ;¿ä3JJZ¿Û¹69y¿ÁíõçMWAGNbll1RXS J033514.5-445929?ïÿ¾"ìý>þæ•™†?~ÀÞN>þæ•™F?ïôúýx ?d\ø™¾°?V
Ù¾v?d\ø™¾²?ïƸ®ÿ?y-Ӏå?|£üz(€¨?y-Ӏå?ïÿõ"‡>ې"ç…D>ÕÆ×Øðê_>ې"çy'3FGL J0336.5+3210@cã@¢‡À2ß?@‡¯ŒÀ8¥ÎÆ¢aÀ;£êUt?ð"éŒùM@†GqD@ÿ•!¿éÅÉjý
¿é—£‰â¿ï50ZÞj¿ïöZNÍdðAGNfsrqNRAO 140?ïôw—Qô-?aÑÌ]·!5?WÑ\¦D?aÑÌ]·!6?ì‰Øòñ´Ø?Åò
"l?»±8hrY<?Åò
"l'?îbòŒ
Ý0?"5.¥½?©Ð×?",ø?"5.¥¹?æ€õ1%«é?·àN*³?Òþ´¨-?·àN*³3FGL J0336.9-3622@mÉõÀv}5ÀJó²ŸúÜ«À:XSy#ØLÀ;ç@Çplz?ãoú¯@Á@«"ªO@}¾€ƒÈø¿ã¡EßL$¿äM՝Î)¿í2išV
¬¿ïÿ¬vÒ*–AGNfsrqPKS 0335-364?ïnrBâ1?µrA¢›%?Œ$coGsª?µrA¢›%?àÇ1ýÞi?щ"Øß	?ÞqœCÏ/?щ"Øß	?ìEZü¹þ?¨l᪡J‡?½Õ/À0?¨l᪡J‡?ÑQ»­A<F?¹Ê¬¾P›?çW")_aÞ?¹Ê¬¾P›3FGL J0336.9-1304@i+eà.©aÀHr¶?¯À9÷×fƒÂ˜À;Ͳ¿-?¾ÔT1Qÿ@
I—è¥#@\ 2e¿çœX¸uIP¿è
LTþp¿ì,í4‡'Q¿Û Kb\ŸAGNfsrqPKS 0334-131?ïñ?ãz?_Ú(ý
Ïm?]õç€9È?_Ú(ý
Ï?ï×ÜI0{¼?ÊâÅÝ/p?tÛgÂ";?ÊâÅÝ/r?î÷l25J?'øPƒFeb? ‡é<Ü«f?'øPƒFe^?î|ôõ^!?¤ÐDï´P!?¯0°ªé?¤ÐDï´P"3FGL J0338.1-2443@k\_x5œÀJNVßà¥ÈÀ:Ç×-xßÀ;Çå–È.?qê™*üµ@µ
a½_G?ô"=!±í?çÚ«»ÁGð?îàÃdCK"?Þ²~àä9"¿¼y¤Ëj¼AGNbll1RXS J033810.1-244337?ïý—(™À?C4üþØOÎ?7ËF»2
¯?C4üþØOæ?ïóÎ(æ÷?d$ñ‰[ۈ?Xc¯Ð2™?d$ñ‰[ۇ?î®n±+&Æ?›´ƒL»™¨?¥íM"¨?›´ƒL»™¨?ïü•*'I?Cž­	«??;WήÅş?Cž­	«X3FGL J0338.5+1303@e±ú€Ïž8À@uç_ö	ÝÀ9R&"©x4À;+_ùdÛL?ãyc)?@M<yØÞÿ?û'Àä6K?ÿ
¿ÀpÎ^È7g¿×ë´Š¥z¿Ü
{ÐA1µAGNbcuRX J0338.4+1302?ïø|qžR?Lï.å?N9ù†·M?Lï.Ô?ïÜ2É×½?wØÁi:3r?qæ›!~¾?wØÁi:3s?ïQ=\Nû??"óº3,?•ÍøTv b??"óº3'?ï '—jNÞ?ŒÂ®w·ag?›û
¶$q?ŒÂ®w·ah3FGL J0339.2-1738@j\¿ôw6ÀI"l?Ä;.À9µè«î0À;Âóá?âEz°AÉ@§¤d"ê;?þÙeÿä&[¿³ó€çWMÖ¿åù25Ý1Ÿ¿ÑÞh_S¼Y¿áɱD00ŸAGNbcuPKS 0336-177?ïý¿Õ\…ð?+ï×L5?2UЃ?+ï×L5b?ïí=…Øc?h=Æ@}?bÂzb'œV?h=Æ@}?ï#Ç?… Ì6ë	?ˆ¾w?¸–?… Ì6ë
?ïf€Ãš1Ð?N~ JL?"/猹Æ"?N~ JK3FGL J0339.5-0146@g€À
¡©ÀE9…¿ÈŒÀ7êûgPÀ;Ao¸õs?ø
ÃÁ
w@1sHL@«,Tò œ¿âBü÷Àt¿æ=ä²F¹£¿æË°ŒÇ›'¿îB"¼díAGNfsrqPKS 0336-01?ïÙÐSLCˆ?n$á],R?sÖYÞ<>?n$á],R?ïñÍÉF"ä?f¯8¶£ÿQ?\dmrØ8&?f¯8¶£ÿO?î]Ëþ¥/?×ÌS?ª'ã@­?×ÌS?ïôë Œþ?X­èæ†5?Wè)¾æ~?X­èæ†<3FGL J0340.3+4130@c9 _ñØÀ&;¹ÿkÀ8‡"õÎNÀ;YnÉw-@shÁ_†@qÁ:Gz?úAÔ£ÿÏ¿Ð$ð¿ßî¿Ïéx¬0—o¿â"‰ü²\x¿ê;õ2,ßPSRPSRPSR J0340+4130?ªr#–±?¨{¶ü=zî?îXÝÎ6"ï?¨{¶ü=zí?uäè±Aõ?¤ëîÂÎý?ïÔ6.}Æ?¤ëîÂÎþ?²MýÖU¦P?¬}tÇ'Q+?í¶@E5K5?¬}tÇ'Q*?"öþ2Y¢Ä?we…bmU?ï¬$6™t?we…bmU3FGL J0340.5-2119@j¹ fèlÀI—Ï¿ÆT
À9¨¹t*tHÀ;ƺ_ÿ¿Ó"(h@!͌Fµ@½j?¹ÔM¿æîNm)Þ¿Ø22ä{7¿ç§›ãõi¿çuê	k)AGNbllPKS 0338-214?ïôW²>Y€?Wí6Gz'?WP›ƒLü/?Wí6Gz—?ïîEïŽbl?m£';é?aºq"'?m£';ê?ïdÔR-?'ãB"‰'Ù?œ3}åuº{?'ãB"‰'Ú?ïàpºÎœš?f×O©`j?oE1cc¾?f×O©`f3FGL J0342.2+3857@cu¨ÙºÀ)¡ÃA2Ð7À9c2:å¯À;sƒY¼3ø¿í$GÎÜؚ@8rP)Ž@ôR?gôÜ¿äSõCŸ£/¿é%©K­¿ß6Á¡å1¿á	pe)
ÌAGNfsrqGB6 J0342+3858?ïÿÛý(>ñ ÃÝÁ¾>òkùü5q>ñ ÃÝÁÏ?ïԜZhZ>?Å;žîKð?u±ÒËÒá?Å;žîKð?ïã¥}Xu~?q¨jdŽD?lZ'§ŠZ?q¨jdŽH?ïÿÑڌ`h>öIçvŠ>÷¹ÏËÍj>öIçvc3FGL J0342.6-3006@l|¡A(¿ÀJCr_˜ìËÀ:Ûk3TÁ"À<?'æFñ¿æmŸÐÀLa@ދÞðæ²?ý‡_úfŽ?ïÿd"$©>¿ç¡jé?¥d'qya¿ãÈï˲ùðAGNbcuPKS 0340-302?ïÿ™¯ÆËY?
™1w›¶?	"M)ý?
™1wš¿?ïñîcÙ?hµÔG#í?]ÙÐ#8R?hµÔG#é?(Ž‰œ?ƒßìõÃáK?ŠšµÜ]˜è?ƒßìõÃáJ?ïýI"?7{+–ìL?7Õ·&ëy?7{+–ìs3FGL J0343.2-2534@k"$?åÉÀIÓ½ÿªo«À9dïS	'À;Áozân?õIu"¼gÐ@ÝŽ<_@z®YÒY¿à«îz
vë¿æ™,¡É"Ý¿î\+~LÐØ¿ï夦Î;AGNfsrqPKS 0341-256?ï÷¥3R€?S€§[]x'?PÞµ™Zþ?S€§[]xŽ?ïðêÐ9?hSˋg3?_ÝÂ*_'?hSˋg3?í¯®­áëÕ?¢,K˜õS?²'Šð¡[?¢,K˜õS?_x¹?ƒù‹²¡¦(?Šy(!ÑÆ?ƒù‹²¡¦'3FGL J0343.3-6443@qsb¯È°ÀEԛ æÀ9fÖ 2¥oÀ;´UhaQ¿ÖYÛ¬AD¡@ÌÝÚçÐ@;}ßÔ¼Z¿Î² yL¿æh»j—¿Ül3,۳οåÿ3¶AGNbcuPMN J0343-6442?ïÿ´ »:õ?B€¿;>ù?×Ñ1BÞæ?B€¿;>Ò?ïïéя'—?k0h³-P?`.pØi?k0h³-P?ï«C3vŽ?…œ0~ä':?…/3"\|Õ?…œ0~ä'7?ïö*zÍZ'?L"©ªt?S«
eK´n?L"©ª`3FGL J0343.3+3622@c°ƒÀ~à±À-fLÿyÀ9Õáƒ=6ÂÀ;x?ǖ,'ÀXî$`\Œ@ßE	¬§@i0`¿çWœ=Q³ì¿çޔiÂ7¿áÌøàÀ¹]¿ÝyHª­óAGNbcuOE 367?ïùÔî[«Ô?S_¤\ÂÒË?H¬F'P·
?S_¤\ÂÒÐ?ïҁr
ê?'Tò‡._¼?võ¿Fú‹?'Tò‡._¼?ïS薲ì?¹w©¾?•'í)¿b'?¹w©½?ïÿEjg·º?"%çŽâ¤n?R³	©?"%çŽâ¤"3FGL J0345.1-2353@kEi_ªŠƒÀIm|_Ìï1À9Bn
Ÿ–3À;ªªùš‹?æé»áJ»Ä@{Ú\S=@CU_'òc¿âýږ‡Ì¿æë)ʏí¿æ2ًn€¿åš\Y""BAGNbllNVSS J034518-235218?ï̙φsJ?{ò_–t?y³<ÆZ·?{ò_–t?來9èÈÚ?"ßÂÕÞ'/?†Ô±…ÍÉ=?"ßÂÕÞ'.?íu~UâÌ?¦°,«¨qŸ?´TåPé¯?¦°,«¨q ?ê<ÇUÚ'¾?¯ÈŸ;ïã?Ç⨗a?¯ÈŸ;ïã3FGL J0348.6-2748@l1~þáÀIr¬¿ç<À:ëWÒNíÀ;ÒþÈÈ[N¿œ@2 îÊê@ƒg5™?@6Ÿú0Þ¿æxxi?¬
¿ã›åGO¿ã¹Ý³h¼q¿ïÿÛå:úAGNfsrqPKS 0346-27?ïìz$&¦S?iÂæÓ4"8?c…ÛÙY­Û?iÂæÓ4"6?ï…ÍÜC>H?˜&^¶±?ŽŒˆï0mË?˜&^¶±?í¦ÌÊü÷™?¥¤ŽSºIú?²É™¨C9?¥¤ŽSºIù?î}!à"£¥?™<MS˜¨x?¨-á÷µÅ³?™<MS˜¨x3FGL J0348.7-1606@iè¾ß¤?æÀGË <¶jÀ9wÅüÀ;Ä	Ñ:×?çt[5}2@ڗ.u0@»#à)¿àx7YáÀ¿ç'fÈHr¿è2ee4¿åH6¿H™'AGNbllPKS 0346-163?ïøƒ
ûF1?O
)¾?ŒÂ?MóÔç:Ñ?O
)¾?Œ®?ïÙ@Üø"?€á0Ãl,?s_'÷ƒ¾'?€á0Ãl,?î°HLÇn‰?™Ó˜K­1?¤û{3‰m?™Ó˜K­1?ìñ=Ãò
‹?¨yÄi'ø?¸vào"¤?¨yÄi'ø3FGL J0349.2-1158@i<c>ÿPÀFÞ-ÿ틉À:.¶(E™gÀ;¤¬§"W`¿Ó7‹¼%#•@Qð/¨d8?ûÀ
ÿ±¿äW̍ÀP¿Ã1®õ\Ÿ$?¼~=Ù»ƒà¿Ø䢃šv0AGNbll1ES 0347-121?ïþ®ˆ)¼?'+NÄn˜?%}d?ÖÅ?'+NÄnc?ïôgÈFÁ?dYÓò9M,?Vß0or|Ö?dYÓò9M*?ïΜ¥†£?u-Vý±¼?x±÷­<­å?u-Vý±¼ˆ?ïü÷·î?6Ò—†ì(?8BGè‡?6Ò—†ì3FGL J0349.9-2102@jÌ¡ á÷×ÀHƒ-••À8ÅQa£ÊÀ;Ÿ>øcSŒ?û¨:üÖ)î@í-(­Z@Þé	nh¾¿àzZá;Þl¿èù›âÊ¿ëòPË°©<¿ïù¤ë¡#AGNfsrqPKS 0347-211?ïæɺoÍ?e̦Êq?i6E2€r?e̦Êq?ïï8©íE?ióð—ɳ?`ÇâVº¤?ióð—ɺ?íe=Ôv&f?¥!ÏCç·;?´Ö\NÌÅ?¥!ÏCç·>?ï·|ÛU{ó?€¹ì¢?' É*¡?€¹ì¢
3FGL J0351.1+0128@g[@îÙÀCÍÿÒ³—À:qbBë7À;‡»DLÊ¿r4G9b
@
›mrÊ!ø@r*ßý ¿â®õ惿éì¸
Ú
¿îùW'8&b?éM°&±AGNssrqTXS 0348+013?ïûC‹/Ø2?P‹çöT?BñÓ@Ÿ:_?P‹çö_?ïí]¡Ò(¥?kËFê?b¢^-×ZR?kËFæ?îÊ×³Ó ?"{Š,…è?£_"ÂÎ?"{Š,…ç?ïó7={ÜN?dMcJܒá?Y'…Gc?dMcJܒà3FGL J0352.9+5655@b9ø -à@½¾`Mr¥À9¿aY·+{À;j¥.ùÏ?è
~A4¹×@
ßôA…ÜM?ýT@ÿ¤n?é_{Ò£[?ïú¼3Cñ"¿â2	6¬Üº¿Ù£}`Ül[AGNbcuGB6 J0353+5654?ï]ÉpGä?ðÀoŸ?"FÑ÷#?ðÀoŸ?åi†…`|?Ôⷁï?Õ-úòõ??Ôⷁï?íó)ÇÃã? RÝ\VË)?°gƱÁàí? RÝ\VË)?èQf7
^?À¶Ü.þמ?λþg#ʊ?À¶Ü.þמ3FGL J0353.0-3622@mÄô@¯¹ÀIUøØþ3À:w™Á݅'À;®0Ô´!Û?¶aš
¸	@Ì<C¨ p?øÚu!??Ü¿ïÿVëQж?ïýÍ«øty¿ÐGЬ³ÛB¿Ê'H/wDŽAGNbllXRS J0353-3623?ïÿexË?zvcÕK?óPækq?zvcÕP?ïñî®ß¤Ú?iÿi£Šó?\"¢@¶KS?iÿi£Šú?ïÁòÚÔrÊ?}ØQ"¡Êg?'•Æ›?}ØQ"¡Êg?ïócs…)?UŸ±¯¶?Y9Âõ¯?UŸ±¯¯3FGL J0353.0-6831@q¬' ÄeÀDcX R…ßÀ:;Äõgö‰À;­…¨K
E?°QÔ
°g@
èlXï
?ùÑ°Ÿ¶5¿ã?^…zˆ¿Ýå‰ïNú0¿àì7¶(¢?¢¨´"œ¯¤AGNbllPKS 0352-686?ïüÞÒDœó?5rÍrÕ°ä?9	mÛt•?5rÍrÕ°ñ?ïð€:§›?fß]º?^äÿŠ°Ê]?fß]¶?ï'Ò(…?‡J͏¸?‹ºKuúžë?‡J͏¸?ïì¨0¨?])?J>l?cWÏïçXµ?])?J>n3FGL J0354.1+4643@cGŸfb5À«
–ìÀ9·ß(ë²À;Y
W—Õ¿'ÙK•'"f@iÆ@ì"M@
ä?Z2ü¿â'¸…¼Ì¿çÏNK+f¿â¶ë±`Ø¿æSZ¨m
AGNbcuB3 0350+465?ïó«Šz؏?_+•Â–tâ?X¨ë
Ná²?_+•Â–tõ?îÒJQU‰È?®ŠJ›p?¢ÛZê§cu?®ŠJ›p?ïoã5 
	?Œ`®¤Î\
?'™Kþ¾Ð?Œ`®¤Î\?ïe{¾y}?'è˜P…?"]0ˆ0ÐT?'è˜P"3FGL J0354.6+8011@`Lþ?5Ÿõ@4¥_ yˆÀ9†mpEã9À;ٞÞ|øy¿âùͶט@Ld×pä@ü?_'`¿åÝë«_>Õ¿ä>ñ5'g¿äN­i"¿é ä´AGNbllS5 0346+80?ïþ…ÅÛfB?*õq«8]«?'£¢I›Ý"?*õq«8]‡?ïâ³ óÅH?xºþ½ñ0ð?mL_:¸Ô?xºþ½ñ0ñ?´ÐŽ?Œ1JAºly?ŒWÿÒËܲ?Œ1JAºlt?ïÿï~ÊXc>èLòv#¹ê>à5§l,>èLòv#·ó3FGL J0356.3-6948@q¿÷À*ýÛÀCéUÿæՍÀ:C|»<'À;ßÀãŠ~tÀlÌìW@U<µ'ôd@<šà–ƒ:¿èúJÉÒÇc¿×Ù­w"œ¿ïÿ׶µ´,?ï÷7ã=ŸAGNbcuPMN J0357-6948?ïõ5ŽXÈ?fhÈSW?U"ãOr¸?fhÈSZ?ïó͚iŠ5?b¡óÜ?XdË,ë™a?b¡óÜ?îç™ö&3?›·d#äA?§†`œÜ?›·d#äB?ïÿÿ
ùïì>¬H"72>ž ÂlnŒ>¬H"7œ3FGL J0357.1+2325@ehß½jYÀ6ppCßÀ9ü³1ñÔÀ;˜Ûmy€¿ß>^Κ@
¦•°ÖÍ@JÀŒ}¿äÆî–Ì	Ù¿ì—Õ°\¿Í™Sƒ_Æd¿Þ='7äYAGNbcuMG3 J035721+2319?ïþێCT?$‡:Jkf›?"G«ÊÈÛ?$‡:Jkg?ïà|ûÆƒ?wŽþC!Ê?oƒ~9}›?wŽþC!Ë?ï¨Ü†Ù
?'Ài~hF`?…ÈÞI¹¼ã?'Ài~hFZ?ï÷XØ2?Hñ¶-°î?QNOé›Ö1?Hñ¶-°ÿ3FGL J0357.1-4957@p+i€,
JÀHb`GhtÀ:+à¤&À;ù)CÆ(nÀE¦}X@V†´åzn@DŽ*GQ¿Ý!Œ@hâ¿åwºXáA¿Ù¤ZŽ}¿à¬$vAGNbllPKS 0355-500?ïÿ¨%ýh?¬¢gœÐ´?ö€¥øÚ?¬¢gœÐ•?ïóöß«N?c8ëÏX¾¦?Xâ@©cñ?c8ëÏX¾§?ï¼[«0¿ù?gü¹­?€é3ÐÎ?gü¹«?ïÿô7u4>â ]õÑF,>בû—rœ>â ]õÑK·3FGL J0357.9+3206@dX6m
JÀ/ù£~õ©eÀ7q=Y&ãÀ;="Ö¼@üFØ
@ñˆ\…g@"Bè\ö¿ÒJÿ5]c¿ã(vÛmhR¿ì§nœJW¿ïj?©¹!tPSRPSRLAT PSR J0357+3205?F¡eɦ?IS$ÛöêÒ?ïúW¼ &Ž?IS$ÛöêÒ?`3Î-4·?kmššS?ïïÌï1ÒÌ?kmššS?…Þ֑ ´?÷É~Sä¯?ï«è"¥¹}?÷É~Sä©>üs»9	ö/?H&*¶E?ïÿljì?H&*¶E3FGL J0358.7+0633@fê}æOUÀ@Çk 	ŠÃÀ9EçbzH›À;s® 9[k?Ütëüà2R@ØJl4܁@É •¿ãþÚ®ŒÅÌ¿é9Y¤e£¿ãu5ÀØß¿ïÿqtâUAGNbcuPMN J0358+0629?ïÿ¬YG?	IHSØi¥?é®:»­Ñ?	IHSØj3?ïàÂn‡tL?vËÃB)º?o='x‹´]?vËÃB)¼?ïž|Íäã8?"ôA#žQ?ˆ`̆Ç2-?"ôA#žQ?ï–m"ål?zù¸
U?Šd›¤ÜB?zù¸
S3FGL J0358.8+6002@bàP7P@è‡@%´ðÀ9…З]À;Nâ~ú?Ý3ÑÏÒ!@)ðÐq@$ˆÿÃo+¿ãØÑÂ؃¿è²‰"p	¿ã‹·	RJa¿îXQúøÄAGNfsrqTXS 0354+599?ïøݒ&ȇ?HDðn§gÏ?L‰·dÝçs?HDðn§gÂ?ïÀ¥Ù‹@?ÒTq¹Í}?õ-:_Ã?ÒTq¹Í~?î̍à·rv?—ç©C«
³?£7!ôˆØ¥?—ç©C«
´?ïô'¿w*?S2ñ½‰2\?Wòځ­$?S2ñ½‰2l3FGL J0359.3-2612@kØädIVÀH!'	±À:"QN"¹À;Û4̐fë?Ó½I¬ÇHÔ@
Y9Ìö@Œ4ÿf'&¿è‡-á7¿é£¤"ƒç¿Ó‰J†áÛþ¿æHðLÙ¢AGNbllPKS 0357-264?ïþ⨡?%Ûú	H?!Õ~•îéŒ?%Ûú	g?ïÜz,(â?{‹à!ŒH?qÂéõëŽ<?{‹à!ŒF?ï}.øƒ?Š±ÈHÞ
@?\Z=@ïv?Š±ÈHÞ
E?îÇ>Y̔½?—ÜâŒ^ìE?£Œc6´8?—ÜâŒ^ìE3FGL J0401.4+2109@emÌÀ7"À7UH¿ŒrjÀ9˖‹È¿À;‹³ß•ý-?îjÌÌÒJ@á㇤N©@ω REr¿â½¨ë¿áŽ"Ç̀ô¿åœ,4ÖZ¿ïÿ4`tAGNfsrqTXS 0358+210?Â>Ùû¥)J?ĄÒ•*"?ëpIµ®?ĄÒ•*"?½®P9BFÒ?¼œôÛÀ?ìJ5ø×·&?¼œôÛ¿?àS?#»lz?¾,s©!¥Ò?ßY¸‰'?¾,s©!¥Ó?&Þ_­?¢KŸ½à?ë~¶Hh?¢KŸ½à3FGL J0401.8-3144@lå7?1n7ÀHN‡à3±ÞÀ:V"ú¾À;ò·1Z?²åäÃ0
[@}ù?œx@J‡™xb¿è"Ûs¿çÔÔxñ6¿Ö¢}›Ǩ¿ë-:¾AïAGNfsrqPKS 0400-319?ïýdŽf:?5 é½%Æ?4یÎ/ã|?5 é½%Æ?ïãzM½Ìú?ts$úÞÞÕ?l…²B3=?ts$úÞÞÕ?ï"é,‰T'?†g FszÅ?ŽÅ´ÝªÛ?†g FszÃ?ïe×E: ?…Ç[×,lï?"E]ø¬1?…Ç[×,lì3FGL J0402.1-2618@kä}sÉÀGÓõÀjÀ9ø|]H°À;·ßâSG?åËWw"½ë@‡õ!ªŸ¦@ðX•m?ï2î>âi¿Üc‰¨ÆïN¿çÛ¸M
û¿Þ¿9€:‰AGNbllPKS 0359-264?ïÓßÉ^
-?½è,Ø=Ú?vPúéZ?½è,Ø=Û?精¤áö?•9¢=fB?…Ø–Ç'Xó?•9¢=fC?떝èïÂø?²©"ožòc?Á¥ˆ\@ô ?²©"ožòc?éí/Ë%;?·iîy¯¢?ÈK@Ók£?·iîy¯¢3FGL J0403.7-2442@kž¤_ZÙjÀGzX`fÀ:'ÅÁ?ÐÐÀ;ö2 f<u?¼#$Œ;j@ñÈS{½@ò`À48¿¾–û\_Û¿ë¡ÃBE°õ¿ÞýϦ=cZ¿ïòÂómAGNfsrqTXS 0401-248?ï歔JéŒ?t‰ÑËû7?iRkµt3?t‰ÑËû;?îÜïÉadD?©ʒ-"Ñ?¢1ié»À?©ʒ-"Ò?ìÔ?x‰?¥ãÔéN¥G?¹^;·Gá?¥ãÔéN¥G?ì%"¦/Ú^?®kÔ¸•?¾ÓZ΁-?®kÔ¸–3FGL J0403.9-3604@m·{€©Þ‹ÀH;Ã`<€ºÀ7/.g˜À;>K֘'ª@Žƒ¹Þ^@FG¤5)@¬BIхC¿â¡w¾ji¿è ×ÌOñ¿êPEҔ"S¿íÈ%?¡øÛAGNFSRQPKS 0402-362?ï´¸'[P¹?Žqßu‹N|?'ÑÛi+ÑØ?Žqßu‹N{?ïê;ŠWÇM?ƒUë_|?eÄu¨8²g?ƒUë_|?ìÄ@NÎ@=?ªa»("µ9?¹Ýý‰þ?ªa»("µ9?ïûNòkó?O'EÇã?BÄ7ªP4?O'EÇÿ3FGL J0405.5-1307@i¸ߨq¤ÀER3çüÔÀ9Æ$PA`óÀ;Èi;,ü¸¿ô/Þr¾"@öÉ™"{@Ä<€L¿âËK-ƒyz¿æŸÚ÷e…I¿áa¯Ü7_#¿å³` åÏcAGNfsrqPKS 0403-13?ïÿïÕr
">Û­VŒmܟ>à*òjþþ>Û­VŒm×U?ïó¤õíŠÅ?cšb86œú?X¶$êv ?cšb86œü?ïï|.Âÿ6?ePH°²w¿?`ƒÑ=ʈ?ePH°²w·?ïÿlن'?ÿa´û?¤Éž_K€?ÿaµó3FGL J0407.1-3825@n(*Á	J,ÀGìè_ÐJ0À8î÷™ÿñÀ; ÓµZ?ð¡R¥ê4è@õ5`Šz@.âôV¿âŸaþü¿æ=U?;n¿åp»ÝøTv¿ë ÂJñIAGNfsrqPKS 0405-385?ïìޜh?b¯Þ-~8Â?c!cú—K?b¯Þ-~8¿?ïê¿Êq,?m)è:Ì`?e@ë5ŽÕi?m)è:Ì[?îçd->èï?"¾VÍö?¡‰½,q"?"¾VÍø?ïŸ9È-x?|LfI
?ˆ>ñô¡Ã?|LfI3FGL J0407.5+0740@fý-`ûHÀ?)£?4É5À9\¨\ªûÂÀ;nNá£1¿ñÕ«}Ç«ü@Dõvºš@…¹'!*¿è®+£4I¿æ…Œ™"r¾¿ë^BØ¿À[{26šAGNbllTXS 0404+075?ïâú§ë R?o—v.æÒ{?mXß­Ô?o—v.æҀ?ïì'ôÌê¼?l÷¢Zµ?c}3D«?l÷¢Zµ?î+^[P¡k?žG@'¸"?­JJõéd?žG@'¸!?ïú½ù»?GÈëZZO?GõŒ'?GÈëZZT3FGL J0409.4+3158@d–]¿Î·‰À,ÎRAtÀ9ÿ°ŸoœÀ;‡yÎøö÷À¢ëý¿‰@S¿[o'@û¨»w¿êX™|ÆØ ¿èžô'%Æ¿ÓN¦Œ-¿ã‹Õe"¼AGNbcuNVSS J040928+320245?ïýjT'Ž1?;:""6B?4­[kŽwy?;:""6Aà?ïÛ(ªú?'Ü—¥Bä?rsü몂Ø?'Ü—¥Bã?ï˜ù^Î?"ö¨³?‰Á½(~Le?"ö¨³ ?ïÿöÎõ]‡>Þ6$XÐý>ÒbDócL>Þ6$XÍ3FGL J0409.8-0358@h{¢ÿ‰;ÀB¯Ø€_5ðÀ9n93't¹À;‡#µîe?ë\˜1e@WtßP)@"< DXŸ¿ÅéÊ A‹]¿àuñ—ë¿âÏòU¿Çx¿àŽ¬£ŒŒ–AGNbllNVSS J040946-040003?ïà@å!LÒ?o7«µZ´?o¿Þ³,Ô?o7«µZ°?ïÊZߚTî?'èÓRo•Q?zҐ2Ո?'èÓRo•O?í¦÷+/ 2?£[T
ç,ˆ?²ÈF¦'þw?£[T
ç,‹?ìχý\äu?¡Uú×_?¹ƒÀÜ_?¡Uú×_3FGL J0413.6-5334@pm#@ˆÊÀFR ÿ¿h`À9:mæÎÀ;¼À2Š–Ç?ÒGp²D¶=@¹Zîu@Ïâ_[/Q¿ä"9¿äEÕwŽà¿éH0s˜ÜŽ¿Â‰,2§¶ØAGNfsrqPMN J0413-5332@?ïþó`]¦?Vªo,? Éÿš%'V?Vªož?ïô¡¯â™û?d[¯Ó5P?V¼ :Ì
ž?d[¯Ó5S?bƒ>U?†bB‹»ð?Ž'_0jÅ?†bB‹»ð?ïÿ]ànu'?ò aÔxA?Cò1O¢Ž?ò aÔxu3FGL J0416.6-1850@jÉ{¼¾bÀE/0ŸÚü:À8þ,"	7À;«kÙlî@¿¬=¨7•c@Á'eé>@¸áß®{Ô¿ä€ÚB×%¿ã
–t 8Z¿è_
Úyˆ­¿áEÀDbDAGNfsrqPKS 0414-189?ïý¬	¸vØ?2Ù ÿ9®Q?2Ÿ²<IER?2Ù ÿ9®W?ïòŸg¯?e•" Z×Æ?ZÁ1ò ÄL?e•" Z×É?ïZAò2€+?‹þD†-	?"·Á¹¯ú¨?‹þD†-?ïùçu½¡?CAvèŒÁá?Hb)	yŽ,?CAvèŒÁó3FGL J0416.8+0104@gúŸDÔEÀ@"п "`À9‡Ûk=À;Wè°X"ÀþHDè<@0:/{Ä?ûë©ÿ˜Q?éW
¥—̿仝‰'&¿ÑmE;Q¿ÐàP7OøfAGNbll1ES 0414+009?ïÿM*
£H?Ÿ´;g+¢?Z¾«–ÞR?Ÿ´;g*é?ïñÍ°–çp?gzkf.ž¾?\džÒ1!!?gzkf.ž»?ï¨_Þ+?ëTK¦4?…è?:Èu?ëTK¦3?ïÿþp©g»>µÝctß[>¨õi"Zµõ>µÝctßB*3FGL J0418.0-0251@h€§ayWÀA"@f!À9#'RÑ^À;‡JaM!ò?ïÇã_û,@=×{ýQz@¯'ÿÏ-¥¿ç'üÏ¿áçй–d0¿épN[$O¿ïÿݹë.ôAGNbcuPKS B0415-029?ïé¢ôªê†?fè8甗¼?f]UyW?fè8甗¿?ï\Q†8¥? !µ÷àö?"uޏ8ë? !µ÷àö?ëDO!¼Ü?¬9…GöA??ÂîÃ{‰"?¬9…GöA??ìE§™‡?¨hFҟ.š?¿-ÒÓ3Â?¨hFҟ.š3FGL J0418.5+3813c@d2`c'À!N·@§[À8סíûñ~À;4'b"s?ð`ãD³c@Ðü&Å£@K7GMœ¿çՆGqD¿ëùt7	'¿èˆ¦0š–^¿ïÿÒ"¢kAGNrdg3C 111 ?ﳝé¶?‰:Ø°'Ë?ƒ½'z?‰:Ø°'Ë?ÒµÑJÁÚ¤?Ð`ºKàè?æ¥ZŸ®?Ð`ºKàè?ëiïouH?²Brô×ò?ÚXBB*Ú?²Brô×ò?֌hNsx?¯äBðÓÍq?ä¹ËØÆCò?¯äBðÓÍq3FGL J0422.1-0642@i@lÚÀBÛíöéÀ9®°E­‰À;¹V¢¤W?易 ûðs@Õ˒@Q†Àyt¿àÖ.½Ø"*¿æ){þS-¿è§´í]&¿äj"]Ú£AGNfsrqPMN J0422-0643?ïÀ¨¥·ZH?~xzm'ÿ?«­$RÛà?~xzm'þ?¹ä|?™~YŠóL?]'†àÛý?™~YŠóL?í	ñ#?ª'¨éhÿÅ?·ô°w^ì?ª'¨éhÿÅ?ê%Ž53?²‰½"¤È?Çiǃ+5?²‰½"¤È3FGL J0423.2-0119@hi#ßm¹AÀ@5ߵݝÀ7‹@ºs,À:îﲪâ—?õºX€õ‰@%@ô¼Õß@ž`‡)T¿á×ù}Ò59¿åwGø<<F¿äÝÌ_¥¾&¿åÃ'Š¼ÂAGNFSRQPKS 0420-01?ïüÈèñ\6?@¾X›«ˆ?9¸¸uWÄ?@¾X›«…?ïëd³ÿp?n`Úø÷ M?d›Lâf?n`Úø÷ J?ïy–/[Ì?‹]gÿOØý?Í:œ&š?‹]gÿOØü?ïø¶dtfh?LмÖÉXæ?M&n.fba?LмÖÉXÙ3FGL J0423.8+4150@cöX@žUÁÀÃßé47À8MQŒ»À:Ú¥ÉRÄÉ?áE9bã@«ØW—V?þC‡¿&›ö¿ä™˜¦eÁ¿ÞãÙ5¿ÌOąÍ×0¿áS#h¹0AGNbll4C +41.11?îýv¾aœ¤? éîOh? ("æ5¶? éîOh?ê
€õšï©?̜¹×"\—?ÇÕü)"A\?̜¹×"\—?í§Ò¬¢ ¨?¥Lú®ws,?²ÁjšêúÉ?¥Lú®ws-?ëýFLº?±ö 6JùS?ÀªæÍí?±ö 6JùS3FGL J0424.7+0035@h2¢iÀ?Ëy`>.9À8'Ld\¡À;Iû_‡O?ÑïdöyÄ@üŠOú"0@•?æ¿Þu—''¿åsÿ©÷h_¿àSwa¥%¿ë/ó
åAGNbllPKS 0422+00?ïü.ä‹o?;á'pM‡Þ??†ˆÛ¤'À?;á'pM‡ß?ïÓ1ø¯.?ƒK"ÁŒ4™?vgü(iy?ƒK"ÁŒ4›?íèg¿{É3?¢ŽYØä[¦?°¼Â!¶k?¢ŽYØä[§?ï¿U'0q²?t¾H"²(?€*›³ã"š?t¾H"²)3FGL J0425.0-5331@pbâ:¸cÀE€ÇßþùÀ9gCÁðÀ;ԝñ.ñ¿õåØõ$.Þ@Ùð5²"g@®ˆ  ^…¿ä¾è$/ùÝ¿äÔ7r2!¿ÜÛpí0£¿ëãAÄלAGNbllPMN J0425-5331?ï竒«?iÕŠ…ßÎ?hTmøoV?iÕŠ…ßÍ?ïì$²#?n¾ÍÞô	?cÛMÜ~ês?n¾ÍÞô?íÿ­ÂW‡?¢¡à
óÍË?°'íGÛÐ?¢¡à
óÍÌ?ïýQ¢i¼?9ªŠ	o8Û?5tì²_?9ªŠ	o8ô3FGL J0425.2+6319@búâ~@#…ïÕ"\À9Â*·c®üÀ;röq?Ù¾9½w*•@Ì~ ïÏ0?ÿme¾Ë­=¿ã—vå˲'¿èç	<Gaœ¿Üf9±~N¿…è¨(0ScAGNbcu1RXS J042523.0+632016?ïü-¤áæÔ?<%iÒöÂÞ?>'ØðÉ\1?<%iÒöÂå?ïȼO<"?"Þ*¤Ò‡Ž?{¡Øaµñý?"Þ*¤Ò‡?ïÅk%Mñ?|Ï;2ýs¸?}JmYv¯?|Ï;2ýs¶?ïÍ4šÒk?rOâ(¸>?yeñ2–É×?rOâ(¸;3FGL J0426.3+6827@a"¦°)(@*°°|À9ǾZCBuÀ;£°Ôcš¿ñ·O,´@ '¯€@Ò@!¿ã1i¼¿è3©a|‹†¿â'7Ín)̿䈺›"=AGNbcu4C +68.05?ïû|¤[D?AÁFx?B
ùn'ð'?AÁFx?ïÚW–ý?|‰µ£0þ?rþÔ4pî?|‰µ£1?ï¶û¿¹B?3THµ?'¯"?3TH¸?ïõ²¨ü+?UtS"5ÀŠ?Tš®©Ô?UtS"5À3FGL J0426.6+0459@gµq'lÀ<î™?׆dÀ9RöT…"À;T"K"bÑ?'Šò˜Ö~'@°Ü{š*@q1ßöö¿åxŸú쵿çê_5UÞj¿æDªøÍÂÒ¿é>!'}AGNbcu4C +04.15?ïøJø¦'Ÿ?Rµ£u¹%I?NÔeµ…õ?Rµ£u¹%T?ïÖN½ü2"?:t,ò?tØ¡涠?:t,ñ?îðIGd<?›.S÷gŸ? ûnۉ¼C?›.S÷gŸ?ïq±¿\C?2-wŠw?'߉Èw?2-wŠw3FGL J0427.3-3900@nEg!éBÀEöŽ€`ãpÀ8»rƒ«ËÀ;AHð3Ú"?æ"Uö_Jò@¿%oü^@`;»²¿áÿfyJˆ~¿éç±(Ó"¿çµ'"?W¿ïÿGýUçÏAGNbcuPMN J0427-3900?ïþÅ4£+?)ßxõ¨ö8?#¯LµÍLÒ?)ßxõ¨ö^?ïêÜ?b9?p‰ýÁ0Ñä?e#ÀäƉ?p‰ýÁ0Ñà?ïIa¦££?$Üá=°?–ÓË+‹ª?$Üá=°?ï'@'çÌ?n£¤³‹‡?oû[F
L?n£¤³‹‡3FGL J0428.6-3756@n‡?úÁÓÀEÏàaÕÀ6jˆû¼¤aÀ:3Ám9Í?ù˜ðN²»@õØ •ŒD?þe@å£]¿Ü},ÈØC¿áC,ú¨¿ßì>{¿äŠI2à
XAGNbllPKS 0426-380?ïÞ—×?tŽC?ú(å?pñž´{"ò?tŽC?ú(å?ïòTB§ç?hë&!ô?[Wûz°2o?hë&!ô?í¸C}?ç?¥lÆ¢1§?²=äÆÃ?¥lÆ¢1§œ?ïÿörË_>ÞEÙ#›|M>ÓäiE¡>ÞEÙ#›…3FGL J0429.8+2843@eG¯ ×{|À*ôUÿøÀ9¹õÞ>YÀ;W'2ÂÊë?òÿÞÇöú@ZM{³Õ…?ÿiE pÝ¿ïœø¦ÅQ-?ít:!ín6¿ÛÏY*Nï¿ãf pMoõAGNbcuMG2 J042948+2843?ïmùƒ?"·˜þÇ?'@ßÝÏ ?"·˜þÇ?îJh%?¸ÆÐ&ú"?¯˜ûY}º?¸ÆÐ&ú"Ž?êÅêæ–û?¯¸xÂóH?ÄêTe¤?¯¸xÂóI?êK¤æ±±?¶K'÷\Ü?ÆÑlg¹9;?¶K'÷\Ü3FGL J0430.2-2508@kóóà7ÝÀD "?Åè­À:•mºîÀ;Ï¥·µ
"?²v_ÛA`œ@­•ÇÒçï@‹ïà"?¿Ï#.LË¿áR»<	N;¿ç¿oA+n¿áq'ÝëXAGNbllPMN J0430-2507?ïِíÿ‰?¿:žÇ?s7ù‰;n?¿:žÆ?ï즎êp?mËÛ³5²?cYåq¦?mËÛ³5±?îI:¹r[?¡¶í®˜?«lThÚOi?¡¶í®˜?ï¥ÿ|³ˆL?ypÛ©4_P?†€ Óí	?ypÛ©4_P3FGL J0430.5+1655@fxV[åÚÀ5ªKÀ9B«×‰¿1À;NaŸWH¼¿á®ÅÁHh@Ò&Œ'@6†@ €¿äêG‹H·Ä¿ìRþ]Ï¥+¿ÍéY¨ñXü¿ÛšÝl"AGNbcuMG1 J043022+1655?ïþÖrl›?(z±g?"˜Þ)6OC?(z±gw?ïãH êý?v!ð*q4?l·ß÷C?v!ð*q3?ï¦r]Ä?€qa«¹?~¬ÆÑôí?€qa«¶?ïý¥"µ0?0Jÿµ?2Ó_ºVyê?0Jÿµ3FGL J0431.6+7403@a``þG™@1\w·À9±{£aÀ;¿Á§ÕœÀfºó±h@
±Šî0×?ÿÐNI¿¾‡*…~sg¿ãš+Œ°a¿Ûf¿ÕÌ€¿Ú@`"ú¯oAGNbcuGB6 J0431+7403?ïóqq½¹?\™71íZâ?Y"U?\™71íZÝ?ï݅¤+%?{egÀµx&?q=-êmsp?{egÀµx(?ïW=òiÀi?ŽC"Ý""s?•A²Çòü?ŽC"Ý""h?ïÿ{š´w2?½cQ²?Œ©qÂÓ?½cQï3FGL J0433.1+3228@dûá`؇ìÀ$Þܾ²W×À9ôwa`m(À;ûý<a¿ÛM¹ë¸d$@eýua+?ÿ~5?|푿äq#mÑG¿Ö¸ŒÃпàDe°¼~¿ÊÛk‰n†ÏAGNbcuNVSS J043307+322840?ïø£*—Ý2?N»³-&yè?MsU ‹;¦?N»³-&yê?ï—BUÿŒ{?˜Cýh,0?Š/j€àÙ?˜Cýh,0?ï²Y…"Ê?€L–¤`?ƒx©žžÍ‹?€L–¤\?ïù!!Ö?D—ã/Â~0?Kÿ{{¨y?D—ã/Â~"3FGL J0433.6+2905@eQŸÛÒúÀ)3UÿæՍÀ7胦MàÀ:ÑñËu?æ(Äwò3@Vmrõ@+&`;ÿà¿Øk®h¢p¿â-ôT"¿à+=ðÈÌÚ¿ßÎЇ\$AGNbllMG2 J043337+2905?ïüÿ–x%w?8ѐ˜?8L>ÔE=?8ѐ˜f?ïÉ¡¿ýn£?†ÕÈsbõ?{/ H®"?†ÕÈsbõ?ïzÏ6ÖQ?Œ¯ÁmÄ?¦%5Î2?Œ¯ÁmÇ?ïõ¸7Dt?N@`;ˆÔM?T'w«?N@`;ˆÔA3FGL J0433.7-6028@pí_ôöÀD'ï¤hÀ9*ÜÇÔÀ;É'o°'?ãód»|ª@æ'M@–?Çì¿Ý&â k¿æ$³­ZÛ]¿èØ7»x¿ïþÏë݀œAGNbcuPKS 0432-606?ïýf×Û-?5¶qãªû³?4ωA&œÖ?5¶qãªûä?ïïÈzÇäè?h‹Ô‡ ã`?`7…8­?h‹Ô‡ ãb?ìn-?™Hœ¾?¤•ñ?	?™Hœ¾?ï÷¹Ü‰×?IڗÈG§?PŒFìPÅÇ?IڗÈG©3FGL J0434.0-5726@p¯ 6mÀDq™_·ö|À9óÁ¯bYÀ;ٔ¦ë'´¿ªù[?ÿç@'Ùv©T£?ÿú•ÀF+³¿ç;áVûi¿Èx½Òš'o¿äX"ƒv±¿Òé`VVúAGNbcuSUMSS J043344-572613?ïýï	ғ©?8ʁ0sF?0‡±kbµt?8ʁ0sEõ?ïîÞÆG5ß?jÐÏB'\˜?a!9¸Ê i?jÐÏB'\•?ïsyb¡}?ŽVO{òH?'pÓ«Ðf?ŽVO{ò@?ïà4Sʈ?f}µä‡ä?oˬï5wG?f}µä‡ä3FGL J0434.0-2010@k8
¿cíÀCx–@HÅlÀ9×
bY'lÀ;Å
ÎÜd?ðz8ËxŽÝ@m³Òê@–!@l³?ïù\œQôƒ¿Þ³4²‡¿æõb!£ò¿ê#£7AGNbllTXS 0431-203?åL ¶á˜?ÊBÊlœ–??Õgɾ'<Ð?ÊBÊlœ–??í=³Js?ºïæ_8š?¶e¯<gC?ºïæ_8™?Üq6UØG?½G£~b4O?áÿGdÕÜ?½G£~b4O?âÚ£G@z?¼™ˆ+ˆž?ÚJ¹Óq
?¼™ˆ+ˆž3FGL J0434.4-2341@kć rѯÀCõöÿ¦=íÀ9ø*/~rÍÀ;Ш•µßJ?äèþ®òf@{'Õ‡ÜX@ÃÛËÍH¿à>+•ì¿èæÈtVÉ¿ãÿ©²&¿n¿ääµ
_AGNbcuPMN J0434-2342?ïñ^{¥°$?bwknør?]C´Ÿµ¨?bwknøt?סּÂ4Ý?ŽZ$松?"Ÿz²ÈÔ?ŽZ$松?îM¾ž=š?¡Å
¸å?«$Œ&f?¡Å
¸å?ëšT£çÓ?¨î['7?Á—ú­p`¯?¨î['73FGL J0434.6+0921@g^­@ªêûÀ8Ë@—ŸÄÀ9Í
eÀNÀ;‰pà<ìÀQ4MdŒÇ@&`ú–´@êè CZ¿ç™ØÕTìӿُW¿Ûu#¨¦§Ê¿èÔ;D_ç'AGNbcuTXS 0431+092?ïè*Uœ‰?jC[1À?gðÕªcv?jC[1¾?ïåg÷Pê6?xà0NQÍ®?j˜¯ʺ?xà0NQÍ®?îؽXäº
?œN($½&?¢t*q´_I?œN($½'?ïÿ}OÌDé?Î%£¸'?Vwbãg?Î%£¸™3FGL J0437.2-4713@o«˜€"åÖÀDüsßË­À8¿qw; ÀÀ;Àîû.	@šõº+àY@	«¼üK@ø/M˜w¿Ò´JÀ²¤¿är>Y_ W¿ë·D)Јï¿íĬ妸fPSRPSRPSR J0437-4715?eWyÂ[ÀÎ?eçbʽ?ïꨆ=¤??eçbʽ?z]hÃäN?'ç¢1v³?ïËçE.x7?'ç¢1v³?²>ݑ²?¢±›ßkBp?í¸<ðMÉ?¢±›ßkBp?œþŽãvð?.S3'…?ïÿcˆå?.S3'…3FGL J0438.3-1258@j;4 -œñÀAª(CìÀ:/rq6¤À;ÀlÄNy¿Ó'èxWˆ0@ú¥>hp'@Ù f|â¿ÞAš»>¿çÒúdúDn¿°pN$XØg¿ëV°j¸ÒçAGNfsrqPKS 0436-129?ïñòm"?p™pîM7æ?]ô%ÆÚ?p™pîM7æ?ïâ_à-  ?s-!?m Ò__È?s-#?î'Ì5õA†?›®ëãð?§Ó< «ç?›®ëãð?ïâJúL՜?qv·P;c©?mµ³*cý?qv·P;cª3FGL J0438.8-4519@oY._ú;›ÀDåù jn3À9?ÖbwÄ]À;¾s"LS?ëÅ`ûK@^d‡éîÇ@!¥?êüŽ¿â¿®{¿äpqÎ_°%¿è
žªÁ¿æÀVò!'nAGNbllPKS 0437-454?ïu¿Q¤'×?"V0!"0|?'HËm¥=?"V0!"0|?îÈ~´9?¨­ˆç¹èK?£x"¼f?¨­ˆç¹èJ?ëd»-3å?­c
§(?ÂoÍK0q?­c
§)?æPÃjI"µ?»i¯…Å•?Ó^y+mº–?»i¯…Å•3FGL J0439.6-3159@m"†_•'ÍÀDZ{Q^—À:fùû@ýÀ;ÆõPy•¿ùh80)1@ÅB' Ôa?üT}?ñ²Š¿ïý¨é²z€?ïýÎ'üÚm¿éDúöÄå?ÆÁOòlÕ§AGNbcu1RXS J043931.4-320045?ïùh_R³ý?PXŽK"'y?J^'µ0Ÿ?PXŽK"''?ïò‹]lÂÜ?e´S%R'?ZéE&zE4?e´S%R'?îÿ›¸¬mÆ?"£úÿbȪ? Du9#§?"£úÿbȨ?ïÿP÷V3'?‡àKŠ	?á9šó¢?‡àKŠ…3FGL J0439.9-1859@k(¿;ê'ÀB $€	À9Õ~ŽÑ¿À;ª7Pþ¿õ'óžá@f' 'ìÚ?þµá)¦¿çÀØˑA¿á>š'LËá¿Ú¨—Êr»›¿Ý¸7´¢3œAGNbcuPMN J0439-1900?ïÿ"è`®ü?
 ûÁ@M?
ÅçÔA Ò?
 ûÁ?6?ïïæ:hùÛ?i˜¬'ª,¶?`ŗ$?i˜¬'ª,¶?ïÚ†i•?q'Èjç?rÿ¼Ë5}
?q'ÈjÝ?ïÿ/Áä[?f1›AÝ?ßãt•æ?f1›AÝ*3FGL J0440.3-2500@lT2TçÀCÿ·äÀ:ԕ(ñÑÀ;í(åÒWP?êìãZON>@yAôl#?û–×6&-¿ïþ~ôãÓ`?ïþÒúb¿²@gÏ2f¿éölš:²AGNbllRBS 0570?î2SÓ÷Å?²ÎU³ãæ1?¬ÚÂÀŽ£Ç?²ÎU³ãæ1?獏Ɛb?Ò`ªƒázÆ?ÐäàsÔß<?Ò`ªƒázÆ?ê[Ú"ig?±®"J##ô?Ɛ—vYÂ_?±®"J##õ?è^ً…Ç?Ã-°÷Íö?΄™Ó•èæ?Ã-°÷Íö3FGL J0440.3+1444@fåw'þLÀ4zƒ?»òÀ9WIáËa"À;Ip:$¾ü?â
!÷N@]E€gÄ@(k 7™¿àh•ž?ú¿æn¦ü®'οèºçC_j
¿á ¢Ç둉AGNbcuTXS 0437+145?èë7í¢×l?Æ÷‰!¨ðA?ÌS It¢P?Æ÷‰!¨ðB?íÔʀÓsG?»¾èъw˜?±Y«ùdeÆ?»¾èъw˜?è"6€
ºÚ?¸aÛHÓ¥?ͯ%ÿÉ™?¸aÛHÓ¥?èqH["\?²È,—PC?Î:ßΓv'?²È,—PC3FGL J0440.8+2751@e'@¿ã°À(h> Ìÿ"À9È£¥¦îÀ;oW6Gºª¿Í
à6i§@2ƒÄ›%
?ÿ0/}HÖ¿Þ^ëì*h½¿é
M`äyð¿Å³Ï¿Š2ã¿á±¾™XV-AGNbllB2 0437+27B?ïûùrüs?G"›P)?@42?G"›P,?ï¾('¯·Å?Ž¯ëÈ/¹¥?€u۔V?Ž¯ëÈ/¹£?望™#Æ»?C\³O1³?…[·Q–?C\³O1´?ïê»aðoü?`»/	 ?eDžå?`»/	Ÿû3FGL J0442.6-0017@h¦€Ÿb0wÀ<vŽ ¿"(À7±åvø…À;EŒ^G³ô?çÒ4oý@»O)@÷Íÿ§Ày¿äê/ô^'¿çÜ+0ý›¿æÃÔ;è¿ë›‹¤•¡AGNfsrqPKS 0440-00?ïóœ|…»Û?Y»thÕHL?XÇôˆG&?Y»thÕHD?ïëÿ™#?p~¸6Ê9?düüfÞî?p~¸6Ê;?îÓÝY@ºõ?™µªí—–?¢Â*kôP²?™µªí—™?ïÿV}|Ç? 
Cá|o?0Pg:? 
Cá|nê3FGL J0444.5+3425@dþÊ€àÀyU E…EÀ9æoD[y£À;O®²0?à3-;Cð<@¦|«ø@wÈ_ÂX¿ Ôrªä¼û¿áýò?¼È¿åQeà7@¿ê½ZÅÑäAGNbcuB2 0441+34?àsž†ÛA"?ÍT"ₙ?ßÂòI|÷?ÍT"ₙ?ìË];
³?Á!Oæ"?¹¥#÷ªk?Á!Oæ"?æsù0¼yÁ?¶J³‹(?Ó
ž‡}?¶J³‹(?ìxÜ=0–÷?¢å\Šnç?¼9{HE?¢å\Šnæ3FGL J0444.6-6012@pàŒ€AÀCs`ûH
À:\f('ðÀ;ïë‹Ô´ù¿òaohی@^©WQËz?ÿ™¾×ü¿î#ߜ]?Áh%£8æ¿à•€œêÔA¿Ö7‹~ñ*AGNfsrqPMN J0444-6014?ïþÒ6ð'?-¬°ëvÌ×?"ܐÿñ?-¬°ëv̬?ïðÑ!'j?h9M	ñ¢?_Ø]¼û-?h9M	ñ ?ï¼+´¯?z­"åŒs'?€õÿ8Ü?z­"åŒs?ïþ[*‰²J?)),>Çá?*MWdÛZƒ?)),>Çþ3FGL J0447.8-2119@kŽ± ‹ü"ÀB!ÕߛªÀ:Q˜y*À;ÉlËu±?ÄhÔÏ>…æ@GrÄm­­@`¡ ¤$ã¿äY@í ¿ç֗4u¹§¿åÍ‹gb÷¿ïÿ{j£ýAGNfsrqPKS 0446-212?ïû†üÑ?C—jy½Ëƒ?Aåø"¿?C—jy½Ë'?™÷ŒS?±6¨°Jƒ?¥•Ö`‡:Ç?±6¨°Jƒ?ïNÍé?'¯n:Ú|"?¶&^ÞË?'¯n:Ú|'?ìnBn«?§?'*Ô¦?¼ï»"Š¨?§?'*Ô¦3FGL J0448.6-1632@jà»ÿŠ;ÀA6¿Ý/ñÀ9AÞíwÀ;\ä
[2V¿àÉ`í¼Â¥@'_?ý¶¤^ïy ¿ÅÜpGª¿Ýˆ_ãý4¿Õ»Ö[åÚ¿àXU¨9UÈAGNbllRBS 0589?ïý#"êE?5æ¦É¥by?6ãg­Ò³?5æ¦É¥bG?ïëKÈ{™?n{jVŅ3?d´7"fèr?n{jVŅ4?ƒÓ¢"?‡Ž6Óð'?‹ž_[C?‡Ž6Óð)?ïõè¥aû	?Púlo˜?T.µ<	í:?Púlo–3FGL J0449.0+1121@gm ìt2À4ª_ºz»À7䨮àR¼À;:ŠE–ã?ý€qÅ?9Ò@¾‡d¸¼@¼³Ž7eÈ¿âFWÔ8 ¿éU;)]Ê¿è[•'ïx–¿êÙèögêAGNfsrqPKS 0446+11?ïμêf¶4?€ÕC¾"²T?x¡ŠÌ¤åÛ?€ÕC¾"²T?ïq¦s5Å?¡ûJÐb?'Ë1™\‡l?¡ûJÐb?í½´ðÌ?¢–U'œðÑ?²÷rXy£?¢–U'œðÓ?í‰e­¯ª‹?«
•vñ3X?³´Ò''«¢?«
•vñ3X3FGL J0449.4-4350@oΠwmÀCôäàõÀ6Ñd‰"—À:Léki¦?åÅ~Ä¢@Á]Z¤k?ý•\ ¿Ó•¿ÜFž†#¬>¿Ýs䧯޿؉k?$iR¿Ü+ƒÆAGNbllPKS 0447-439?ïÚ¯ÜÍ?~©Í'
êy?r¨}ý˜?~©Í'
êx?ïó1Œ'N?båçl"µ?Yœçû±b?båçl"µ…?î}|_Z? ú[ÌB¨ª?¨.Nè:
j? ú[ÌB¨©?ïó3Ý[tÆ?UP2;?Y˜EIu/?UP2;"3FGL J0453.2-2808@l¡i@5z5ÀB'HàC¢À8iüybÂmÀ;ŸüJhÙÞ?ôPBàÐ9ê@ÓÇ©¢PL@
€€mùƒ¿å`tԊ¨²¿èýhæÉM;¿éf¢®7­¹¿ìá£ÙŽ|/AGNfsrqPKS 0451-28?ïôVò
°?Tœ1T6I?WRÅä¢~?Tœ1T6I&?ïÐt~T?ˆ Ee?~7ÅÀ¹V?ˆ Ee?î¡âž#Û{?—ðeð‹S7?¥áÖÂH[?—ðeð‹S7?î
Z"Áí­?£%¸fs
?¯ZV³á%+?£%¸fs
3FGL J0453.2+6321@bNO€Ü3r@(Y?µ!µÀ9v(ßóÀ;[‡æï?âEi™KÀô@'–E&@Æj?Žá/¿ç¨8_å:N¿ç⪬]ãØ¿Þ²~UNÅ¿ÛÀŠ0'flAGNbcuNVSS J045312+632117?ïüÜÄ24P?7µ
Gb?9Þn]v[?7µ
Gaü?ïÅPD_ª?†¸°¶¤?}{×ÝÐ+?†¸°¶£?ﳈ£`Üo?ƒ,BðÑ(¬?ƒ×'Èä?ƒ,BðÑ(©?ïnŠ'‰\?€þmp©³?'.­Îޔ€?€þmp©´3FGL J0454.6-6825@qzw@=ݱÀAÚÁÀ)P[À9óLŸÀ;ª>"E]?욆 \p2@ðÑ›¯ô@"ä %\¿ãƒ"^ϙ¿äJRŸ	E#¿âB;¿┿ïÿ¸èz0OTHERpwnPWN G279.8-35.8?ïvò`½@y?¥a›Ç2lŸ?'!³èWðî?¥a›Ç2lž?љ'"8û?Ͳéd/ûƒ?ç3>½ã'}?Ͳéd/û'?åe£X{:?·µ[L(?Õ4¹ÁO	‹?·µ[L)?ËÁÛ9Ÿë?´Š5ƒ,m°?é‰1˜=?´Š5ƒ,m°3FGL J0455.7-4617@o¼@ŽÉÀCi·?œÎÀ8Ÿ>õÀ;¡1$e:?ï.9Ķ˜@ßqBn=@^àAHË¿å^WµYÏ»¿èBs'‹ò׿çw'&Ç¿é¢AcÖßAGNfsrqPKS 0454-46?ïý=¸ä9Ý?1wÛðâV?68Þ1ä?1wÛðâ{?ïÆ›²J?‡ñ×té—?|þö²&Úß?‡ñ×té—?ïu=&?‰6ø]Vq]?'Mýþ˜[(?‰6ø]Vq]?îvÊ Ë? Ì]dké?®"]þ£J? Ì]dké3FGL J0456.3+2702@eì&?šIÃÀ$ÔHµ{À8෋òçêÀ;-hÁŠyk?ñYžqŕ @Q¸Ð¢@®i t)¿àʵ4D¿èAÐ…h¿åP‹¿¼C¿ì8ÒXõ1AGNbcuMG2 J045613+2702?︌Wœç1?…rFfbºo?ÜêÆ3^?…rFfbºp?ëˆÓôH?Ä¥nZRPÖ?ÁÜ°/ßîà?Ä¥nZRPÖ?ì˼ÿ´é³?¨@ü—ÓN?¹¢X²e?¨@ü—ÓO?ë
'ó­Ní?¨É-ùºö?ÃÕ´1JÄI?¨É-ùº÷3FGL J0456.3-3131@m+VŸIÀB½¿é{À9ΈJ¼½À;æHEéï?áX쒇N
@㹯c°T@MbÀi'¿ã
ºægÊâ¿ç©¿ê;Gª¿è1Nˆ	Š¿ïÿãï—ìµAGNfsrqPMN J0456-3135?ïÿÆßÄZ?¬¸Û©OÕ>üüҗs?¬¸Û©P%?ï«È4W·?ŽfUYÝû?…
òê;O?ŽfUYÝÿ?ï¾µézÏ?|µ¥ÂlŠ¨?€z'…¡LÉ?|µ¥ÂlŠ³?îEì
ìP?˜ÓI/¼I?«¡?!?;?˜ÓI/¼J3FGL J0457.0-2324@kö©Ÿ¡—ÀAr–¿Ê…ËÀ6uQ'ÑÀ:£º¤¬S@–íw'2È@ Ïryð@à"@¿7ä¿ÞÎmЁҿäQÍ_™Ã‹¿å–À™¿éxŽûAGNFSRQPKS 0454-234?ï|ø[µr?¡ÌD0˜ng?ž0`ô‰Q»?¡ÌD0˜ng?ïìtSf#C?v±ßibÁ?c‹¬™Ü¼W?v±ßibÀ?é«õ݉Q?±¨ÍSÉ
~?ÉSü(‰Úº?±¨ÍSÉ
?ïÿ¸Þç?vŽ»*[ß?È[û…â??vŽ»*[®3FGL J0457.0+0643@hDàÚ ËÀ5°cÀ™¸£À9ämBùyÔÀ;r#QA;¿ÿzr·Ø@ÎÆQ@a:ÿZh¬¿é ?Ðû[¿ãu&ǃÑu¿ìù×bä¿¶õÅÿÔ0AGNfsrq4C +06.21?ïØq­V??€'ÿcÁÒH?sÇ)T÷a]?€'ÿcÁÒI?ïåžE<Ø?w`՚¥
?jaºÃ'â™?w`՚¥?ïþ8eì™?'ï‡
O	?8óBl×?'ï‡
O?ïÿÞâÚZ@>÷dlONä >ðŽ'Òßà\>÷dlONæü3FGL J0500.3+5237@ctÙ_í¦a@e©ÿî7VÀ9h ƒ-FŠÀ;]€
|ZÄ¿Ó`…'F§ë@
[¿Pã@Ë àJX¿âæ=@¿ëD8>4îõ¿Ýa'Èýµ¿Ø—ÁREG2OTHERspp?ïò«5?ý?cϏˆ5?œ?Z¨ß•€×?cϏˆ5?œ?ï©Ê‡¨¿?•<ß?…yžÐ
?•<ß?îɊ́Ҩ?˜°YúD‹À?£gS'âՃ?˜°YúD‹¾?ï²$÷í6×?y6ЄZ	"?ƒv²J7?y6ЄZ	'3FGL J0501.2-0157@i.
á'6À9E  œWºÀ81dÒèoÁÀ;Zl ºŠ«?óÿ2ªøÈ@³¬wâÆ@OB?ë}g¿ã÷|k¿ä¿æ@àùˆ¿å¥\jÓ¿éñ•S0KAGNfsrqS3 0458-02?ïõÅBÓ£l?O.KÄ~kÂ?TuzX¹&ø?O.KÄ~kÍ?ïÞ´ÙAÙä?y@€–¡¦ž?p¥"_
Y?y@€–¡¦œ?ï"œûŽõ?"lms`,E?›¬} Ž!E?"lms`,C?ïöË*Pì?PGb.Í¡?RiÝ«^(Â?PGb.Í£3FGL J0501.8+3046@e¤(?NÊhÀ5pÿÇuöÀ9Íøí½]À;WQ§'€¡¿ÈW%«¶&Ã@ÃɃl0«@þÿÝp^¿Öfm†¯ö¿éíq—
â̿췋aiô³?æÉǓkÆçAGNbcu1RXS J050140.8+304831?ï¼&@$ºÂ?‡hÃ[°·e?€öoöÑO©?‡hÃ[°·e?ïd-ÇH"?¤F¤uU@ò?"úGûÕ?¤F¤uU@ñ?í:nñP'×?¦6ó°Vƀ?¶,ˆu{q>?¦6ó°Vƀ?ïû`Üó&d?IEÕ")èÑ?B|Œ3fn)?IEÕ")èÎ3FGL J0502.5+0612@h>ìß&k¥À4Ó>¿XpÀ9ƒÂl º‹À;'ÅPÉ?¬î"É€[@µž´5§,@¥¹ß_K•¿áS¯¸пì4k‹>b¿áÁÄ|àë¿ïúÕ	öè™AGNfsrqPKS 0459+060?ï92*ÔÆ? Å­È Yt?˜Ù¼z¥g;? Å­È Ys?ï˜
þͼ?©0µ)°g?žþ &H}?©0µ)°g?ëü [‰¹?®«±JˆÁ4?À~'Û‰"?®«±JˆÁ7?î
Ì­¶_á?¢–*)!Ü?¯#5$šò?¢–*)!Ü3FGL J0502.7+3438@eD¼@ŽÉÀ:ƒ?»òÀ93u@ô¼ÖÀ;=KË°m?ìN–ž×@èÆUå9Ö@JL`€É>¿áÿVÛ6¥Œ¿àKTš¿'¿è:¼¢ï>ù¿äû¹*>ÔAGNbcuMG2 J050234+3436?ï«ç5ڝ?Ö­~*?…2‰X¹Ÿ?Ö­~)?îºî{OÉö?²ðk%?¤QK`›?²ðk%?í?zJk?¢aN¨³?¶-«§Á?¢aN¨³?ï¯tfœÝ?w{¦Wb e?""üfXÈò?w{¦Wb d3FGL J0503.4+4522@d7  ôØ@¯rú6<À98‹ò)ôÀ;3>iȶ?jÐì1»@˹ÕÁ@á€.¹|¿ÚÁFíá¿íqÑcµ\¿¹õ¯ÞÄ4è¿áO.+AGNbcu1RXS J050339.8+451715?ïþØó(¼?%˜§?"~0Ít/Å?%˜®?ïIo)]÷ó?«"òŒ±?–ÒÔA‡?«"òŒ±?ïNÁ!|«ž?"~iDþ4ñ?–'ÛÐjŒ`?"~iDþ4õ?ïó܅WB?TŠÎ0<æW?XFõQã{0?TŠÎ0<æT3FGL J0503.5+6538@b'Î ‰ãC@,Ñeaƒ¨—À:X4õ«hÀ;ÇPܑeî?Äà5Á¿å@.ûJ¹@®h@0FÅ¿éqÏÔÐ7¢¿Úü›Ö׿ì[
'ÁË?Ù£@'ªAGNbll1E 0458.1+6530?ïoE¨¯[ñ?".ƒ±_Û?'JêØ?".ƒ±_Û?ïÕ¯rܹ?~éS–ïï?u(F'£~p?~éS–ïï?î9hÕàð?¢H)EœÛ?¬ir¡ÿô?¢H)EœÛ ?ïÜLqÛ¶è?r+…Î}ñ¶?qÙÇ$‹÷?r+…Î}ñ´3FGL J0505.3+0459@ho0_®¼AÀ4ÜW?öÀ86ÈqyŽÀ:ô÷eýŠÛ?ûaܶ#é@ób–x'@Ïï=*¿á½Ë"Ú¿æ@*†!¨Ø¿éT‰;Ÿá¿è?nO"æýAGNfsrqPKS 0502+049?ïÛ ý…èâ?pP*)?r/=Ž‹?pP*)?ïۏ$æé?zBqcˆ[ç?r8m¿‹Ä?zBqcˆ[ê?îK:·îåb?í§~?«LT©þ?í§|?ïõ\XñϦ?U'ÔÒ¾ŸO?UGN`µ¨?U'ÔÒ¾ŸJ3FGL J0505.3-0422@iŠsÿ¬*À9…Üßi‡ƒÀ9Лx–ê"À;pæDm[?ó[
/')@
֕Î]ñx@
ú`-è¿ÚeÙµàÄs¿ä˾mA*¿çÏé°Äi¸¿ê™¸õˆAGNfsrqS3 0503-04?±9râ8?¶ëÓ/_8?íØÑ¿¸?¶ëÓ/_8?Þ<¶à†Ž?ÔT–¡?àᤏõ<º?ÔT–¡?ÏÆ,Ä4?´†®,M?ètÎÿ}ô?´†®,L?Á‡pJ#ñ?¦¤6ӔBÊ?ëœ#íw?¦¤6ӔBÊ3FGL J0505.5+0416@h…Ÿj"óÀ54"Ÿ^ÕxÀ9Џº–iÀ;vVO—íÈ?ÒG»_ç5@<OM:?þ}q +Y?ÝÕ«:"]¿Ñõ¿èÁS¿¦FöLпäHMÌ#1AGNbllMG1 J050533+0415?ï!­œ?˜ŽþWvB?Œ7ºø˜ç?˜ŽþWvB?ïE ¼¯ÁÙ? «?òHT®?—KèjÄø? «?òHT­?ï8E©‹E¨?ìE<¹P?˜÷JΗK?ìE<¹O?îÒ"s‰?—3J½4?¢ßÈÇo?—3J½43FGL J0505.5-1558@k&€IRÀ>uàè@À:7œÓ	ý°À;͵±þm¿àšŽX•9Û@
2"¤Åœ­@ÐúÀP»¿×'ƒk7¿ábvs5¿ç •—‰ýx¿Ð[±e¬ñÕAGNbcuTXS 0503-160?ï96-ó?¡
˜Qw?˜Ù:Ažý/?¡
˜Qx?ïã%t='ö?u[éQëó?lڋÂØ
r?u[éQëô?ì΂]èǟ?¬Yóõ$"?¹‹í¹Ã?¬Yóõ$"?ïÖ|ô`:?p±…æÞ‡?tÁ…Ïâòí?p±…æÞˆ3FGL J0505.9+6114@b¢¸¾øγ@(0¶â—À:òÿf}À; ºö
´¿ñçêc5¯@(
e‰œ¡@;À n ?ìŠb=(¿é¬l'zk¿¸'eŠzº¿å5¯CéAGNbllNVSS J050558+611336?ïÿC.L˜â?ÿž{wc?š6l㴀?ÿž{v½?ïáúD"Sn?xBjZ'»ÿ?n»k¬'â?xBjZ'¼?ïÅÙ~Ú/Ë?{#¸17Ûá?}@'èR?{#¸17Ûç?ïþ¹E6?)'ÅD†?$o;¬Ÿ¡~?)'ÅD†I3FGL J0506.9-5435@pf¸À>-ÀBbë@UZ¥À9n?"zM¤À;P9Ø?çÅ
uÀf@ð»"k1?ù¥Ã P­m¿î[þ÷tô§?ÇÁXXg?²W\PT¿ØÞR—bÄAGNbcu1ES 0505-546?ïíKåT'?_òпŒã?b´û«n*?_òпŒç?ïÙå
uov?y'½½Þî'?s
zÅHD–?y'½½Þî†?îØOãùlý?•ìž'÷x¼?¢{Ài0?•ìž'÷x¹?îç^AUÌ? vbç"Z?¡Šê®ã@? vbç"Z3FGL J0507.1-6102@pæ}ÀTïFÀBtߥíeÀ8ä(í_ŒÀ;ª3Ž¢Å'¿nyJè³=@ü^h–'@%ҟʋ)¿ç¬DScv¿¿åý '®¿çøbí¥¿éø^i¨÷AAGNfsrqPKS 0506-61?ïþÑùrߤ?#v¥Yæè4?"àhÒÀ?#v¥Yæè`?ïê'ì
(5?q>:€@ø?enõ×Ê??q>:€@û?ïqÃèR"8?s›ò¦Þ?'Ç'õ­™?s›ò¦ß?ïô>©Š`ñ?Si¼í#kï?W'¬ë>V?Si¼í#ká3FGL J0508.0+6736@aùÖ`^åi@/È)?"j†À8CÕAæÀ:¿Œž"#¿Ï'Ÿã	Ð@lŠQýù–?ø]q?ˆV%¿¡âe+ÓÿἋw¤¿¿ÃlJÎQÕ¿ É^¶ÍAGNbll1ES 0502+675?ïýÄ7eÍ¡?46ê™?1ÞDђïº?46ê™(?ïã!ÂÀ.@?wŠëTÃ?lÞ=?ÑÀ@?wŠëTÃ?ïyJZ'?'`IÁèÚ­?Ö´¿ÝÝ?'`IÁèÚ¬?ïýµ†Ã-Ý?4󰧾…_?2SÉæ'd?4󰧾…=3FGL J0508.2-1936@kŽ(`ܹªÀ?0Üà@GÀ:o4bÞªÀ;ð).ˆª?éK×V5
J@Uµ(Á?P@ÿ^@}¸?ÔdQ^þyS¿áòÆ7‡¿åGQ¯Z¿ïÿf`˜W`AGNbcuPMN J0508-1936?ë°¨³ÿµÜ?»Wî(Y†?Á=]0(•?»Wî(Y‡?è|wÈA¢o?ÈG#ƒ˜³?Î ÞùvD?ÈG#ƒ˜³?è	%㬆É?²
Þeê?ÏÛhqMäÜ?²
Þeë?âÖAÇ<A.?¸4uœ¦Z/?ÚS|q‡}¤?¸4uœ¦Z/3FGL J0509.3+1012@gëý`éNäÀ1?Ê ¢¢WÀ9"Çë¼|À;Vj3z€Ð¿µÐF¦"C@#ȶ@zÎ]=s¿çÂR6ôe¿ç?lkQ÷¿æ3–òí•<¿æÎ8˜ÞïËAGNfsrqPKS 0506+101?ïöUí!&ñ?T"Ð#ŽÆ!?ST%½²8?T"Ð#ŽÆ?6»—?›ÊÍå,¡?‹òQ=Ô?›ÊÍå,¡?ï]['µâ:?ä	Ss–¢?"T©C¸­?ä	Ss–¤?ï…ê"Ÿª?€ûÀ{±+b?Ž…[>˜,?€ûÀ{±+c3FGL J0509.4+0541@hlë têŽÀ3 ¼€NnùÀ7YˆêíÀ:¬ß06)?תŠm+Òl@70BèÞ@Kù€_
ý¿Ü%<`¿š¿â¶‹AèÜ¿ÜNŠê ½¿â-ZfÜ`œAGNbllTXS 0506+056?ïüÎ#"|?;´áîý³u?9ŽãÜðd?;´áîý³?ïÜfg" ?{Üpjâ|?qÌÌ5ò°J?{Üpjây?ï¤Ìï\
g?Œ¥‹=AO?†ÌÄ(ýeÙ?Œ¥‹=AS?ïþ	Yõ/ä?/PÒy‰þ}?/j`­»2?/PÒy‰þd3FGL J0509.7-0400@iæàé´À8gÀÌäJÀ: È{.tˆÀ;«'Ýãu†¿¼á'Ô'¬@
Æà#Á¦?úaäa\?å6y8Ñ¿à$«œ3ð¿–Ä`X™¿´žD—<OÅAGNbll1H 0506-039?ïõ€'ô±ç?\ú|ŸäÄ?TþÜœ4õ?\ú|Ÿä½?ïáÍ£ºYr?w±[Ä	Ñ?n2\E¦‡?w±[Ä	Ñ?ïHú³%Ñ?óA1ç*î?–à¿	›Eö?óA1ç*ð?ïèDÀ:?ehË`Õò?g»û€?ÅN?ehË`Õë3FGL J0509.7-6418@q$·@=ݱÀAš†@ €À: s,G‡À;ä"i·S¿¿Ú4ç
ï$ï@§E¥¦˜0@wœ'"¿éêþí¿ä¦¡H:¿â\:$áXB?µú''JVAGNbcuRBS 0625?ïÿy¥ðÉû?:©œ­e?ËAæÀ"F?:©œ­M?ïî0ÙÃښ?kÓú!ŠçT?aÏ&<%eã?kÓú!ŠçN?ïÖ`	{ǚ?t àÆÎ?tÏûB3+?t àÆÎ?ïüTzœƒæ?9}ƒ›N1?=\+àä?9}ƒ›N"3FGL J0510.0+1802@gû¿"ÿ&À)‡LàƒböÀ8ÀÂã>ÿÀ;7&ùz«?åMƒ2©v@øîÀ½të@F§ msK¿ä¿Ÿ±Fð'¿åîç²è[Z¿ál;ò–ØA¿ë—6Ã5ŸIAGNfsrqPKS 0507+17?ïßù]SÄ¡?vGN{l}¸?pQV®æ?vGN{l}»?ï{ÏBss?•¡Ï›Ð<¢?†±'ŸS?•¡Ï›Ð<¡?î»)_YÖÄ?šÝ¢R??¤Mj
b"È?šÝ¢RA?ï	_H~ß?ŠHëq+ê?žÔð>$?ŠHëq+ë3FGL J0512.2+2918@eõW´Àx=`2Å¥À9®§â1¸àÀ;9WÒNìÍ¿Ûb1ÍF^"@{——᳏@@¿ ¿â@^xõùÜ¿ã2»!1[ ¿ë"j2xοå~¶0u‹AGNbcuB2 0509+29?ïÒs$K3?}6¸Ëp¾?vÆíÚfÝ?}6¸ËpÃ?ï*|Cúí?¬.嬞›?š°w€¼"H?¬.嬞›?î¡ÍTI,9?˜HDË/1¹?¥ã*»m<g?˜HDË/1º?ïàLGוˆ?g÷Žb'œš?o³¸(jw–?g÷Žb'œ˜3FGL J0512.9+4038@dѾÀ//˜?íJ =?ÚÀ9Œ$ôÀ;[a8)<9?è6âGæÒ@"WJê‰÷@͋?cÿäz±|íÄó¿ÖÔ»Ðóo¿âX[œ'¿ãäâ^É'ëAGNbcuB3 0509+406?ï»qE'«E?"ìU0F	[?#®ŸU/?"ìU0F	[?ÝJ9h¤Á9?Ô¾»Òhݙ?áZãK­Ÿd?Ô¾»Òhݙ?íž""9T?¤0Ÿ±¢wü?³£Þî5j?¤0Ÿ±¢wþ?êžÀ–Å<?ª¦Øò>?ńý¥¼ë
?ª¦Øò>3FGL J0514.4+5603@cBß72œ@$»ÁÎjÀ9|5Om&À;}Q›Ô}¿ë¼T2öç@œ,µj°x@·Ñ?Î!6¿è¡ø‹žþ¿éŸã*cÇ¿æƒxÒÇ-¿ãxÓ~ LšAGNfsrqTXS 0510+559	?ïþYÃ\Øë?+uëIA?*cÊ2qZ†?+uëH¡?ïÒ/€jÊî?†ðRO1?vè?ʚ‰?†ðRO1?ï"Àéÿ?†I«:ˤ?‹ŀ9zÌ?†I«:Ë£?ïôʝæ$Ø?TÁsb.G?VjÄ3¶N;?TÁsb.?3FGL J0515.3-4557@ow•@%NÀA¶ó=<¡À:(»ìª¸¦À;›ÕÎÔ
¿©åD²Ÿj@/ÑËdAô@p@.ï,¿éÝ"®Y¿Ö×c©ž¿ç±"£ï×σ3ÒAGNfsrqPKS 0514-459?ëÊ+?f?¼¡†³®Ñì?À×S¿'h?¼¡†³®Ñì?îõw^ÜB?©)‰#"Z‡? ¨Šr;ß?©)‰#"Z‡?é+ùïd"?³a"6kï?ËPøBm±?³a"6kð?í"i1ˆ~?£_Z¥'+?³d³–s¼?£_Z¥'+3FGL J0515.5-0123@iY,Ÿ/ېÀ5Þó_ތéÀ:™`sÞ.À;¸õ½†ß?èkÅd½^@
ch/>\?üÆ`Ìôe?Ôq'ð$b,?æ5ÓL rš¿ÐÙí­Ô¿äy¼*øÉAGNbcuNVSS J051536-012427?|£žH?' ú%så?Ž ×n9?' ú%sä?ìò5KÉT€?¾ž²í'?¸nU¡µ[ö?¾ž²í'?î·Å[Úý?™¨¯Õr¸?¤CªBP8?™¨¯Õr·?éÓžËH§?µã°•ÓCþ?ÉÀ±"ÒÝf?µã°•ÓCþ3FGL J0515.8+1526@gwÿ´€¦À*"ÚA)•ûÀ8Ϋäõ¸~À;.Àp÷Í¿ò±ÞÇ;@$M˜ö\@ŒÐ¿u¡B¿â׳Í2´¿ãtsè/(â¿àèÑÝz;¿Ùø1<ìxAGNbllGB6 J0515+1527?ïúlp>…©?AdG™´'…?FN?é]4?AdG™´'¡?ïÑcaK¯Ð?'p\>º?wNOZ(à?'p\>¼?ïNµ¢ËJæ?'êø'	?–)K¦–£j?'êø'?ïýœ Ú}~?6ÅëÎ?3ù,ò?6ÅëÎ-3FGL J0516.3+7351@aSÊ€à@3Æ"à՘MÀ9ò¯ÑêBÿÀ;ÐùyÔt?òá']
9@‹³÷ñt?ÿu«€vÝØ¿åM¤éXôŽ¿èôA¸Sm¿ÍgrÓº°H¿ÖÊBÐpUAGNbllGB6 J0516+7350?ïïÝMô·Û?]7@éï`?`"²H#?]7@éïf?戴PŸ?8œ­ÉÓw?…xÜëÿWü?8œ­ÉÓy?í%Enf?¥"ÍƆ™»?¶×å×üŒÆ?¥"ÍƆ™»?í<ʚOñ?©²=OWã?¶™«-€p?©²=OWã3FGL J0516.7-6207@pø6ÀP½ˆÀAaG P À8/›fù3]À;JbýüÁ?åãÁ¦(U@pyà@)Á'°—¿ÛN{Òοãhxt…ãÚ¿à–€Ï7$¿æ]º,§ÜAGNbllPKS 0516-621?ïþæàÕ;?Êúmé·?!'óƬH??Êúmé2?ïÙÒ)ôÊ¥?|"«tá?sëš®?|"«tß?ï¡V¨íæ¥?ƒ·8ˆk8?‡ªUĆW6?ƒ·8ˆk6?ï'uÅ[V?}?ÛúŠ½f?‹¢Ž©*~¹?}?ÛúŠ½d3FGL J0517.4+4540@d^\FR@÷QÿÒÊÀ9ËzdJ,tÀ;UÂ%©Ý´¿ä>ÏôEÑ@hú?v¸@°IÀheo¿ç²¥4M¿è¢9`ýN}¿àî«ÌÌ÷À¿è3MU%ÿÍAGNfsrq4C +45.08?ïÿèv‰\ñ>夙ÕÆñH>ç‰v£°ê>夙ÕÆòÚ?ïÑîˆÁ?Š5"à‡ú?wú;ó¬?Š5"à‡ú?ïߗ#=C?sócèíC?p4nax]'?sócèíP?ïÿÆ`›ÑG?ʧÀàÒ>üϲ]o'?ʧÀàC3FGL J0517.5+0902@h0à?pXXÀ0)ÃÀ´–À9Æb‹æR°À:ùŽ,~
¿ä¤¤Ù$R@Ë°…ni@b»q"î?黎W4ÍÆ¿ìñ÷MB·¿Û­ðÂåC¿áä|í͉œAGNfsrqPMN J0517+0858?ïùœÐ†'?b

w[Î?IŒ¿éå¶ç?b

w[Î?ïÈ<›C%.?‡!G8"úž?{á²^mhž?‡!G8"úŸ?íŸDØéª?§öš4QX?³ÕÙ8²´?§öš4QW?ïì¿Wc-U?eÒ.':O†?c@¨œÒª¾?eÒ.':O‰3FGL J0519.2-4542@ooý¿HÌÀA]›ÿ¥g-À:QÈI°MÀ;qÕÉːÀ^+¸ën@R#½Iw@ááÀ¤ËQ¿ãMsjƃ¿è;ԓ¯cŸ¿êÛ¿Z½¶¿Ð²­3KÔ6AGNrdgPictor A?ïývéHC©?:¢Hek¼<?4Hµ½â¼)?:¢Hek¼?ïðƒ¹Ü»n?jjœHÓ5?^øŒF‰#±?jjœHÓ4?ïo¼ÁíáÙ?‡ÞzQív­?'gÂCÄå?‡ÞzQívª?ïÿþ5ÙUï>¶è¤å{O(>¬¢j¡ñ7>¶è¤å{y¡3FGL J0519.3+2746@f:" ³Ô®Àá'_Á0·À9Ó[&—C~À;iï‡â¸¿ôËó @݅6‹,n@¤y¿^¥'¿ìS«lfð¿âö:qÆ}¿ÙÝWu9¿â~'ùZAGNbcu4C +27.15?ïáQOöè?vŒÍ&­?n®°	ãN?vŒÍ&¬?ï3
¸ùi~?¬2b+!?™žHàÒÐ?¬2b+"?c0Fô?œh¾ie?¥5éÌû½?œh¾ia?ïû;ˆì?E¡¦Â%/?CßÐO¯0?E¡¦Â%3FGL J0519.5+0852@h=쿱[WÀ/°¾|§ñÀ99{*BÉ©À;šþô?ùÀZ*ÃÍö@'´#lÂ?ÿﴀ¥¬Í¿Üû¾Ê"¿æWdØi/'¿è?ÀDb¿ïÿ¾ú¤™AGNbcuTXS 0516+087?±ë­GòÁ?²ÐHN–ù?íŠW¼)?²ÐHN–ù?«Î‹Ç<)?µåfÁ@W?îCCŒ?Ž?µåfÁ@W?҇%{, ›?±é¨V0Bó?æ¼mBi¯³?±é¨V0Bô?«dzTRM,?—·£ÃAæ?îI¸ZºÛ,?—·£ÃAæ3FGL J0521.4-1740@kuNóÀ;•sà¢l§À9ÇquŽ!–À;Áó™À0¿ø›«–ò@ÓtMéÄ@nó€jÉx¿âBå'Ñ++¿çѪÒ'¿çi ÙŸŠ¿Üç¶vãÐäAGNfsrqTXS 0519-176?ïô£ºF>?\ZvE-?V¸‹Ás'|?\ZvE-"?ïéû⇨—?pÍ®H‹²P?fxWhÄ?pÍ®H‹²P?ïD [aæZ?xq-Qô?—kô"Ã4Ñ?xq-Qô?ïþ3@?)ü¹,mY	?',Ç«ù>?)ü¹,mXþ3FGL J0521.7+0103@i)rÿÑÜ×À3T‡`±ñÀ:5:¯(wÀ;š#;nk?ÏœÓ+¼@pÁFóµ?û-€H9Ö?îâw]•Ä¿Ó"¨)Ãf—	'›â¿ÇEnbøâAGNbcuNVSS J052140+010257?ïûjû:'?DpcL6«?BT·‹?DpcL6¶?ïʵÏuü(?†ŸÊ…ê»å?z¥Eì<?†ŸÊ…ê»æ?ï¨/}0"±?VtTF{?…ô ³÷Sô?VtTF~?ï÷€Ú±î?EvéÌ?PþJœ#ÈH?EvéÌ3FGL J0521.7+2113@fó'àÀ!gž´JÀ7LªÓ}ÁÀ:l²oStò?Æp^'ê@ëH>³?þĤ_E_Ü¿ÜÙ©Þ¿à
õò"Žp¿Û°Š¡Ú¿ÜSóÉAGNbllTXS 0518+211?ïü8†˜_?DHŒîÊh?>;Ë=á?DHŒîÊV?ïp‹ª­?¡9Gv¶v@?'<ªV?¡9Gv¶v@?ïšÄŸŽ•?ö'Ÿh?‰NØœZÒ?ö'Ÿf?ïþî Bò?1
;\·PÛ?/1ûÐÚã?1
;\·PÄ3FGL J0521.9-3847@ni>_·¼À@­? (ÿÔÀ:?³~G-¼À;Ç?QN§-À¬âF[®ý@^VYS†@… êÚ¿í=ÌÍ´ºn¿áƨR⌿äì~9R`¿à".¾¯SAGNbcuPKS 0520-388?ïÿÔñó>ù1¿øÉF>õóqP>ù1¿øËÈ?ïñ™*ó`@?g«Ôy‡´K?\ͪ?ƒØ?g«Ôy‡´G?ï¼jm¦§?~Öûà¢Ð?€åd¹V?~Öûà¢À?ïÿÿÖRðJ>³œº†Öˆ>tևÚK(F>³œº†Í)3FGL J0522.9-3628@nð`»+»À@[ò¿¥œÝÀ7ë×TLÀ;$†îœ*n?ðZYŠµÑ@æÑZÑ@/hDq¿â§ÝÖº}¿ç8Á5¦\¿ç%]Àƒ¿ä}óKoG¿AGNBCUPKS 0521-36?ïý>"TvS?6zP[K|–?6Ý\Mg"?6zP[K|–?ïíMFº?m£Û¥¶í?b²¹üEqo?m£Û¥¶ë?î ¶"Ó…-?=Ö²??¥ô—²Ç­'?=Ö²??ïýË8¥º?1fєOj­?1§:Ò(4?1fєOjÌ3FGL J0525.3-4558@o}Øÿu–…À@Ùr 0ŒÀ:VHø"À;Ù®&ïX?âÁ©\t	@Ñc	/ª@œôBp¿åØ ¬¿â	õH…Ä"¿×suéOY¿í€±b°qAGNfsrqPKS 0524-460?î_=çÕû?¬*Ö|'%©?ª!ŽB @?¬*Ö|'%©?ïaÒÝé@º?¡
þmGh?"ŤB×è'?¡
þmGg?ëüÿ>y£?²i		¾ë?Ðn?²i		¾ì?íHâGãB?©€új§³?·¸íÀåï?©€új§³3FGL J0525.6-6013@pÑ̀CRÀ@ïÇÿÞrÀ9•üÁ‡mÀ;zšéû±½?ñμI¢á@EpOô4?ûžŒÀmBù¿Òæëˆ
X¿Ü2Ýð-¿"œb2
zi¿áD‰8ð®ÌAGNbcuSUMSS J052542-601341?ïÇÞÖ-›g?ü¤­Þ ?|"é2LÛ?ü¤­Þ"?ïÖ0yÈx?€g}'Až?tçòÃÃÑ?€g}'AŸ?ì‰ëÆ«³—?¨Ó6í‹<?»°¡Ê¢cB?¨Ó6í‹=?î˜cõëße? `/&pú?¦yÀ¡B	¬? `/&pú3FGL J0525.8-2014@kÙq`•l
À;ñ Á¬À:[ìSzÑWÀ;ß:ZMS?–PnU_È@zû¸G¯—@€V@(¿×®éö0üÖ¿á¹u«dš¿×ˆ€º¿èü·•FèaAGNbcuPMN J0525-2010?ïظèP"?€ÀÂÄ6)?s£‹üW·?€ÀÂÄ6(?ïÍÏ°ìÎN?€ó¸rQY?y'‰˜Ù>?€ó¸rQZ?îU±Št¬Ô? -ô…¨ý?ª¤çXµ2È? -ô…¨ú?ïŽÍxܺ?€ÈÅ:ù/°?ŒL¡ûÈџ?€ÈÅ:ù/®3FGL J0526.0+4253@dÔ_õI@Ã×Àâ¯À9\sв4›À;SÕ™êø?òmJ(B>i@óa4Î=æ@{ðà}XÆ¿Ùm¹,˜­¿êzôE•¿åÌ
ÏmÞL¿ïÿàL¨ÇAGNbcuNVSS J052520+425520?áފƊnÿ?Íî¬	 Kt?ÜBêrë"?Íî¬	 Kt?Ì*¼ˆ¯šQ?˾&^È ?èõPÝÔl?˾&^È?Ü5ìxL?¹1%~‰'K?áå	ôÃÙð?¹1%~‰'K?ÇH¼bW1q?ª{zȀë&?ê-Ðçj3¤?ª{zȀë&3FGL J0526.2-4829@oßU>öµÔÀ@àn¿Ñ;ÇÀ8Êû¡ÌnÀ;\¾óÆ5Ú?Ó¼0ýMô@N˜|äG@NR@i§Ž¿âÓ»Ôàu)¿ãÏ¡t?©¿ã"¢3ž¿ç…l1g½:AGNfsrqPKS 0524-485?ïþšŠàv?(GÅ¢·L ?&W^±ø˜
?(GÅ¢·LY?ïìr<sA?m'p<??cÃŒà¿ª?m'p<2?ï'õu¦6?Š¨bƒ+\}?B¢–r_×?Š¨bƒ+\z?ïù¸VÐÑ?A¬¢:5€?I§Ð¼·Ú?A¬¢:5™3FGL J0526.6-6825e@qm~KZÀ@lӀE4½À6_MkÝyÀ:?æW¸Mº?þOI"H¢@èVÁèb@u°Ÿoœ¿ß¾Nî÷ð¿ã7we'+¿å³ß@¿äÂôÁÞ\AOTHERGALLMC?άFŸ­Ô?ɸ˜¶õL?èTîyŠ?ɸ˜¶õL?¢W""'x_?²ºž	?=´?îڇ·½ˆ{?²ºž	?=´?áv€
™"?·Ù±eµ›G?ÝÿåøÌø?·Ù±eµ›G?ó²A?†¶9vÿª?ï€15Âûì?†¶9vÿª3FGL J0526.6+6321@b"™Ÿä6v@.†þ "ofÀ9úÈ×'šÀ;͔ãQs?è
™"GÊç@hfʺMï@Q·fw®¿æâ?j¤
¼¿ãTR+Š·¿ìJªó€&¿ïÿҁWèAGNbcuGB6 J0526+6317?ëƒH馑?Â,dž?ÃõòÜYeÁ?Â,dž?âÿL1I?Ñ?©ÙÕ53?ÛÝègn?Ñ?©ÙÕ53?ëùeÍÜ¡?®˜'»¹?Ðhȍy?®˜'»º?ÓzB%R?·¦Ë>?æBÞùñíV?·¦Ë>3FGL J0528.3+1815@g^·`¿]yÀ"d²—À:s'7ËHhÀ;™;ÞÓ_Ž?æ5P÷¿>Å@qZRÜÆÀ?úU{?Œ?¢eÉæñ勵¿7¿8Sr]¿ÚäP¨u:Ñ¿Æ¡eÑýŠAGNbcu1RXS J052829.6+181657?ï®iӀË?ƒ'X]QA?"e ́?ƒ'X]QA?_-?²–¬ËÇ×b?§åZ
.?\?²–¬ËÇ×b?îîé?VÞ?"ùÂ8;^?¡l
Ÿò,?"ùÂ8;\?îOm²^äµ?&SxÞv»?«	$Ú´™?&SxÞv»3FGL J0529.1+0933@hSvÿ:Þ"À*è¬A<
rÀ9fµ¨ÃÙÀ;DBì䚿æ
·­Å@^&ˆó@ˆÏ`zê¿á[Æi¿çœÏ2å[¿ìY "Qº?×0sêwFwAGNbcuGB6 J0529+0934?ïä+ŠîA?ld
m°–t?kÔéuÀ$?ld
m°–r?ïÓÕïgá?'­ý¾)ÑÏ?v|•Ll?'­ý¾)ÑÍ?î/ÌU'ï:? .zéMN©?­:¦Ña? .zéMN¨?ïþÑ¡x©?'¾©±#?"î…èui?'¾©±M3FGL J0529.2-5917@p¿j€JÀ@½i@5z5À:\(^ÃÚ¶À;Ú`S&ÛSR¦¿@
—>•¼ë-@ÿÜ TsË¿èüî8ég¿åuk—RÂp¿á\6°§cm¿ØSrÇ^AGNbll1RXS J052846.9-592000?ïþ—§Ž©þ?&¢Ê¸æïƒ?&…‡`$8?&¢Ê¸æïl?ïèA¡VJÏ?p~}f­[¨?g¾^©µ0N?p~}f­[¨?ï'ØÕÆì?…âÿð\g÷?‹IùŠŽE?…âÿð\gó?ïæ"êƒ='?bGôàSB?iÝ|ÂØh?bGôàSA3FGL J0529.8-7242@q¼¿šÏúÀ?×ÇÀ'áÀ9«èYM‰À;ªÔ}›6¿úhßè]vÿ@/€3;@ÌπsÝ¿æ^ï_Úí¿ë€ [ՓƿԬ0ÈÓK ¿èü2•ÿ[AGNbcuPKS 0530-727?ïÿúë½Ø>ğìÞäl=>ÄSÅ u¾>ğìÞä{&?ïî ¸'Ay?nl7lL?a_G}¾…–?nl7lD?ïîã­)'?hâeïÅ)?aRþÖ~Í?hâeïÅ?ïÿñ-›ðƒ>詉7F¶Ë>ݤÈøn¹>詉7F»Z3FGL J0530.8+1330@gëü–þµÀ&‹$£MÀ7ºÇªÀ;ÒÎn|?ýËk[BÆÏ@._@B-¡ú¿âúžrœU¿ç—Áf«õV¿èêPⲊ¿í'H¶ÁâRAGNFSRQPKS 0528+134?ïÑ$M+? ºUJK?ŸÅÛZ—? ºUJK?ïywQ?š"#mËÅæ?ßÑÝ©?š"#mËÅæ?ìú¬42i¢?¥œzSé¯ß?¸*ž^l²ð?¥œzSé¯ß?îø ßHV'?š"{w3¡? }òz–Þ?š"{w3¡3FGL J0532.0-4827@oà 6mÀ@g`#VFÀ7F™¦.ÓRÀ:¤"Øi¹?ö¨Y-æ&@0¿»lR?ÿ}•øÛI¿Û¾òˆ¤¿â—:·6¬¿á;—ÇB°e¿å£^™4ç5AGNBCUPMN J0531-4827?ïöw•¯g6?V'\¯°G?SÔ¡1"Í?V'\¯°C?ïï<¼ê?k""I|?`ôçÃC=?k""I~?î÷‡X[œ?•b…³£æ? 7ŠzF=?•b…³£è?ïÿô™Áxù>ạ´aJ©>ÖÌ}Ú>ạ´aAÞ3FGL J0532.7+0732@h›5'Ì÷À+sóþiýËÀ7|äJ7\À:ޖstkã?øVV"÷@ʖpÅ:@¶¤¨ÁTÊ¿á^jL¶"M¿å°?é$h¿ä3Rè°-/¿è6¦¼þàAGNFSRQOG 050?ïçzñ?k¶©ò{Å?h…ûéð-?k¶©ò{Å?ïÓÑîêÂ?ƒ¯ú&ÈD?vøŠŸ¸?ƒ¯ú&ÈE?î݆øöŠ?™lËßÃ?¢'pŸ×d?™lËßÄ?ïûk­N:Þ?A—Ûò÷?BQJǁï?A—Ûò"3FGL J0533.0-3939@n˜¬B»fÀ?d;ߪ#À9îRŠçO/À;¾ê·™^áÀš®ý®í@A
;|Ù@æ½ÿ|¿×¦¾laÓ¿èØKIeµÎ¿æ*EEPäk¿á_"½'"AGNbcuPKS 0531-397?ïýOàQN?B@CÁ?5€ÿeuˆ?B@CÁ?ï@~?k9'1<ú?a}g忁–?k9'1<þ?îëõ€QT?•T=V]B¦?¡O§úêÕ?•T=V]B¤?ïÿð¬WŠ>ç;Rjˆå>Þ§Pê—`>ç;RjŠm3FGL J0533.2+4822@dE$û¨'@ rE AYÀ8uŸÕôÀ;<ERðgÝ?ë¨UTxÛ½@f»ŠPG@__áçç¿âå¬H·˜¢¿å±'ì>hW¿å•™(ýǎ¿çn[b¹fAGNfsrqTXS 0529+483?ïûòÛt€:??•YPGe?@4'-ÿ
??•YPGq?ïºønå7'?'æH§cE?AäF²"?'æH§cE?ïÆ­܉?"	úrÚS™?‡*]¤nÙ?"	úrÚSš?ïÝ_µ
÷–?hôâ Ê 7?qP%z"5'?hôâ Ê <3FGL J0533.6-8323@r|˜`fÀ=&7PþÀ9Xå™LlÀÀ;š¬±¤RZ¿Ë,Ž@'á@æ±÷ßJ(@^*€J¿Øcî‡1¸	¿å\"åX<‹¿çåD¤Ž"¿Ó†fŸNí×AGNfsrqPKS 0541-834?ïþ*`?S?/OxÑ?-Yü
Ï
X?/OxÑÞ?ïëÀÌɝ?o¥["qzÃ?d?3ÿ6b©?o¥["qzÆ?ïŽœÝkR?"¦Ê^h6ß?žn,dR•´?"¦Ê^h6ß?ïÿ-Bvà?T!aéo?N±$F?T!aé3FGL J0534.0+6759@bÄupÅ@22g  ‰xÀ9_UÅ.rÚÀ;¾ÜÛ7ɛ?ù¿y'3J°@`ñz¬¢?þµðØÜö¿ãY©Ìíƒü¿ÖºØª6Ûð¿àEåÝÙ©¿ë}™–ȦPSRPSRPSR J0533+6759?°t¦}eIe?·]AUîí?íñk0SVÓ?·]AUîí?Å!¯Gqb?Ƹéx?î´?귔?®#§?Ƹéx?î´?Ë‹àŠ†??®ÒO¾Z?ëÝ^q?®ÒO¾Y?ŐßK*#è?°V½@Ù\ü?ê›È-5w?°V½@Ù\ü3FGL J0534.5+2201s@g´ßݵÀö@8ªAÀ7®X¡UPÀ9×U,'?
?êy@wƒ3@dN>a@Ý_Ù.…¿ïÿô!O…ú?ïÒj WS¿Ùeށ*7¿ïø¢©Ô$OTHERPWNCrab?â
Éïå?Òþˆ‡!½?Ûêl 5ÃÅ?Òþˆ‡!½?î9'¤¦Š?ÀÜ[›_˜ç?¬gտŗ`?ÀÜ[›_˜ç?å+x£‰5?´mYqí&?Õ©ĸí˜?´mYqí&?ïÈ <âí?Cl¥NH¨?{¯áò‰æ?Cl¥NH§3FGL J0534.5+2201@g¨`ܹªÀ_?«'"À4V8/v~À9D›	Ü!Ô@‹u>›q@»7»ƒ#a@§FÀÙ¤w¿àï÷…nP¿ä'ÛÇ¿å5Ò$O•"¿êÆB9`sÞPSRPSRPSR J0534+2200?èV&x4ƒz?'nTƒô?Χf-ò?'nTƒô?épz÷	±?Ò¡|I Ù?Ê?ö#Ù??Ò¡|I Ù?ä'ýAU?ºÞŒE5vð?×ÕÀú}U?ºÞŒE5vð?âº&Hl%‰?Ï;ÌCYy»?ڋ³o'´í?Ï;ÌCYy¼3FGL J0535.6-2749@lö²ßP]À;ëÃà•®À:oGÆ;À;ÇjM{³Ö¿æ®S+z)@
"½Y'B@Qç_u0"¿ê=:þèÜ¿æóh±´¿äÏ\wWØã¿ÖàüFYxAGNbcuPMN J0535-2751?ïûbwÜÑ'?K½7p"?Bv Œ»e6?K½7p"
?ïæ5:Ð$?rïWMr!?ipÊÅ/Úø?rïWMr!?ïr:H}:µ?ˆEÁ«¯.»?'¸¶ðX©k?ˆEÁ«¯.¿?ï÷£_?Fò¢¦šá?PĸÅËAƒ?Fò¢¦šä3FGL J0537.4-5717@p˜Ô_õIÀ@6ä?°8À:q6Ô¨À;Ûµ_Ƚt?×35/s2@#)@oòä¼®¿ï¬qó''?å+ ¿þˆ1¿Ùé+(]þI¿ß#Ú½GÁAGNbllSUMSS J053748-571828?ïýí
Qô±?4-6é'±?0—•pZqÞ?4-6é'r?ïÚk¶)/)?}2|O/i?rÊ$ëhjÄ?}2|O/h?ïÇ7ms¦Û?{º<b²N?|dIF,'ë?{º<b²P?ïoÑT2ñW?ƒóº!y?'Õy¡Õ.?ƒóº!y3FGL J0538.4-3909@nŽ@îÙÀ>E`IôÀ:SÞKzQÖÀ;Þ|WisaÀf©!¡æD@¹'ùïÔ@S–‡å<¿é	ܘġ¿Õc)%úKÇ¿àðº¤ùk‰¿Ý1*Ê®å[AGNbcuNVSS J053810-390844?ïþâ#tã"?$™—7EÅI?!ÝȱdzM?$™—7EÅ/?ïïC¾!5¯?gÚ¡ƒH…È?`¼AÞÊQÆ?gÚ¡ƒH…Ì?ïÏèJTè?tû	¥Û;?xÚ՞,	?tû	¥Û1?ïÿú¾¾8>ΐ
¥Q·¢>ÅÏû.>ΐ
¥Q«ˆ3FGL J0538.8-4405@oB¨àÉÙÓÀ??Ï"èÀ5æZ¬ôÀ1À:Œáû2;?ùŸu‹ÈJ²@§9Bú?ÿ!L{ƒ®÷¿Û°.fçZ¿áÍ.õk¿á\"ÔvËu¿ã>oAGNBLLPKS 0537-441?ï몿:¹-?nämäó?dU@ÅFÓf?nämäó"?ïïÿÛ35"?iµÃ"¹Ñ†?`$ÌÊj?iµÃ"¹Ñ?ë¾"ÄÜ@?¯šyÁn?Áé°ìŽý?¯šyÁn?ïÿç¯öŸ>öxQû¶4>èP	â_Ï>öxQû·83FGL J0539.8+1434@gófŸê%À!B™`
Ü·À9Wßh°Ã'À;C2Öìá??ò8=-ÝÞÃ@Ìy³JDÈ@'(?7?Í02m¢à¿æ<¯ý»¾¿è­f}bT¿å«þ	rAGNfsrqTXS 0536+145?ïö²þ°Å?XìIßõ2›?Rzšžu?XìIßõ2¨?ïl…(­Þ×? †¥ý^'?'oZêD% ? †¥ý^'?ìêpÆHï¾?¥Í®´.?¸¬y͸'?¥Í®´.?ïñ«+Çf?Y&ùýûÿ?]ò©¨q4?Y&ùýü
3FGL J0540.0-2837@mŸä6vÀ;@>€nOiÀ8ǵƒ+ßÀ;'j&ˆ?í…9Û÷j¹@Äo~)£@:Àß®¦Ç¿æë|ݘ™¿ëÇg©m³H¿çÔr¦™:¿ä½ÁA(AGNfsrqPKS 0537-286?ïþïÜ8ƒ9?ÚëªyNr?!<wÌiM?ÚëªyOc?ïÞ3|'¾è?{šNiŽO?pæAì ‹€?{šNiŽS?ï^Dý࿈?‹*
Š˜^?"7`Cèï?‹*
Š˜^ ?ïÀ'©¯cç?ví"þ?¾«(Na?ví"ü3FGL J0540.3+2756e@f‡ÔŸ"…^¿÷þG€óšÀ7=ò¨(¨–À:"~áS?Òò"|/a©@{pkÍÙg@ŽHÀc1þ¿àÐÜ&$¿äŸ™±Ž¿ßÔ$"ï"¿ç †
 zOTHERSNRS147?äEP"V?ÍÝÓdB³?×Íu^ØÅR?ÍÝÓdB³?Ý؅«{eã?ÔíV4†Tb?á½*BM?ÔíV4†Tb?åT<ûÔ:F?¹V;/J‹ø?ÕW†W‹u?¹V;/J‹ø?êÍP)Çô?½V)z??ÄÊ¿Xà/ò?½V)z@3FGL J0540.4+5823@c=éÀ"š_@,'‹ Z›À9P0uєÀ;€ÍÀÓg?øsÅ@~-'Š[¹@g  ‰x¿êoœß¹¿Ü÷&o!î4¿ÙÿhI¯:Z¿Ý}õ×KñAGNbllGB6 J0540+5823?ïã}¥çä?g‹Ekâ?l'Zÿ?g‹Ekâ?îØ(,P6)?¬Q}%ð:H?¢}}:üz?¬Q}%ð:H?î\%''?ŸÉ82°‹?¯¸
=§Öö?ŸÉ82°Ž?èKýúhæÝ?´Ìjƒ±¤?ÎÐ\dŒ?´Ìjƒ±¥3FGL J0540.5-5416@p_öŸÏ=ÀÀ?ã^è¬À9%Fí$[)À;²u®ØÅÿ?èûµÈEËß@ žæµ,@ãßbüz¿æŽ‹î'¡}¿åឤJ¿ê<:áÛÛ;¿ïÿâÖEé¼AGNfsrqPKS 0539-543?ïþ'Gã5Z?-UŠâè8?'ہ̪T3?-UŠâè8>?ïã!‹hS¢?uÞo'F>ö?lÞt—¬_?uÞo'F>ø?ïi-p\ªK?‰;|(Í؝?'ÚQôj¶¤?‰;|(Íؔ?ïÔµ;·}*?j~³Exê	?u¥b$AkR?j~³Exê
3FGL J0542.2-8737@rÅÈ _ñØÀ;Ð!`¢ØÀ:Þ$
%'À;·ª1—QÁ¿ò×øyùÁ"@LpjKM[@OÄÀ
÷¿ì|_ã{¡¿Å£/ð]¡¿Ê'Õލ¿çô%g~ÐAGNbcuSUMSS J054923-874001?ïý˜‹a†1?3іI÷¢	?3;¤óÎrÙ?3іI÷¡õ?ïè(o¹?q"K±ê
?gאãFq/?q"K±ê?ï°DI\A?'YIiûa?ƒû®í¨ïÏ?'YIiûa¢?ïþ!;͜í?2:‰üoæø?-ìC&1{?2:‰üoæê3FGL J0542.5-0907c@j¬ú D®†À3j矶êÀ9'ï,»À;
I"®P
?ð…««iûœ@£">‹«ð@Š1€€˜í¿æÌî¹9P¿ævx{Ö~ì¿é_}¹
Åx¿ïýÀ~FDAGNbcuPMN J0542-0913)?ëSew‰ƒ?©t9ÊÐõ?²kþ!Ùô?©t9ÊÐõ?åS}Ö¬Á?дÇb'´Ù?ÕYÙR¦~?дÇb'´Ù?æ؊¢ñ«$?¸šç­®c?ÒN꺩¹?¸šç­®c?ە<bÀDq?¹ßeœ?â5aΟÝÈ?¹ßeœ3FGL J0543.9-5531@px+àXšÌÀ?z⟜èÙÀ8œûºöásÀ;bƒ'Öß?Æ{Jï<ŽQ@õ
j?üF·2»?ê¬ï^ñ¿ÕˆÔC¨e(¿Û̓݉w¿Í´˜õ&"AGNbll1RXS J054357.3-553206?ïþÓÜè
?+å¶íß¹?&"Â17?+å¶íß¹†?ïì":ÎC?nzþxâÝ?câlÅ1½±?nzþxâÛ?ï¢Ù6®?ˆ™Óë1Þ?‡I²Tz¬?ˆ™Óë1Þ?ïçߐÓ'"?c\$§·i¢?h o,Øm/?c\$§·i¦3FGL J0550.6-3217@m²€ÿÚ@SÀ:'q_¾¬yÀ:?¢óµnâÀ;›ÔÓ+‹Ÿ¿ä¶Î'¾À@
ØG)_J?ùÖg?Õ-¿èJÙºñØö¿ÕÓòr›x?Â_9è?U<¿à$ÿ³ÿÌTAGNbllPKS 0548-322?ïþ·‹€q?">ê.g\?$‡Gøîlä?">ê.gI?ïæ"D¾´?vn£9ۃÁ?iÝ»AKï?vn£9ۃ¾?ïÆï¼?€‹çqf?|ðùˆ!øe?€‹çqf?ïþàIÖ{‹?$"å*u?!ûb˜GJ@?$"å*«3FGL J0553.5-2036@l8rŸYÌûÀ5¢¡€èTÀ9¤i|›\À;‹"+ÁNê?ò"žÃO£@Œåõè¤ð?ÿÃA`r†…?ïßÉá']à¿ÒW—¡Fâ¿â:.³k¿çñ'‰ÿ?AGNbcuNVSS J055333-203417?ê:³ºr|¢?ÄÿzK0!?Ç16
y?ÄÿzK0!?íù*
?¾ÝÄՎ"¥?·çˆ6¯¯"?¾ÝÄՎ"¥?ä'D3Ý	g?¸àº$aT?Öûw˜Eí0?¸àº$aT?ç
p8™?¶º?'ïÃ?ÑúáåŽÍ?¶º?'ïÃ3FGL J0554.1+3104@fc£ –x}@cý@,À8Çy*ŽIÀ;H5Ċß@ã®:»h@…'.¼!?ú[L¬Öã&?ïã'é9P?¿ß¾W˜\¤¿è¾ÈZÕ¿ïþÊ:Ì.ÂPSRPSRLAT PSR J0554+3107?ÀÆcót?Â.d·#×?ëÿÎg"ÿ?Â.d·#×?D²/žú9—?T˜!ýD2Ö?ïúÓtAq?T˜!ýD2Ö?¾ÁBïeN?°×Ø(æ?ì'×­âW?°×Ø(ç?xóՌ¾?k*_Ê|?ïÎTæƒò?k*_Ê|3FGL J0556.0-4353@oP`=WyÀ<®€±kGÀ9÷ªlO´sÀ;Ê/§î¿ÔaÀê–aV@'…€Þ@œ¸?wT¿Ä»Y¿±RÀ¿àšçg¿è•:í;Ø¿Ô|ÏMIx´AGNbllSUMSS J055618-435146?ï¸ê[¸7m?Žw!ž¹Ð…?Åiò$"?Žw!ž¹Ð'?ïæ4Ëû+?sð`
ÜÇ?iËè4Óã?sð`
ÜÇ?íè!ƒÝ.?¤ÉY¬äm¡?°¾óáޖ?¤ÉY¬äm ?ïëbívcJ?[ÐùeÛb?d‰œ¶1?[ÐùeÛg3FGL J0558.1-3838@n›Í߆ã´À:jÓ_ŽÀ9˜Q`Dä6À;–Å×Eî¿õq»v¹è@
ÞM'Ðÿ?ÿ]É^Ù)R?֋Áýïb,¿ç"	.Ia¿ÍîÉÄ&,‡¿Ú¯‰¿u»AGNbllEXO 0556.4-3838?ïýA.–Ji?:ÿÒºŒó?5ö‹M¬¸_?:ÿÒºŒ?ïåMËNÖà?s¨Vo7y·?j²4±)À?s¨Vo7y¶?ï…Z!¿uH?ˆ¨?êdj?Ž©w"­é?ˆ¨?êde?ïþµoÇÐT?'µ­'}O³?$©'ú¯é?'µ­'}O23FGL J0558.6-7459@qáxÿûÎBÀ=‰ô?Ø]$À9´}C"À;¦üÙÚÒI?⦿aKÁÂ@A<4
Π@oß|&í?íh°HtÛ¿à2‹üU¯¿âda
~U"¿àoŸ"I<yAGNbllPKS 0600-749?ïÜisI#ø?{¤¤@Q¸ú?qËF[nå?{¤¤@Q¸û?ï{N³ë°?™GÖ*›5Ì?Ÿ)'Š?™GÖ*›5Í?î¾
å4õ'?˜23 ¢ž?¤!¬°§?˜23 ¢ž?ì›h÷,Ѳ?©BøÛ`™s?»$¸F™rt?©BøÛ`™s3FGL J0600.9-3943@nź@Ù$À:*Ÿd´µÀ9½
S¥™'À;zòÙ¦Ïã?É÷ù"•ø@g
}†@|­à#¿èHÛúDݳ¿ë»^säåY¿ëÖG¬*ڎ¿ïÿñY/WAGNfsrqPKS 0558-396?ïßIC÷'œ?xZ'ôÏà?p[^l2]?xZ'ôÏâ?ë>¡q¤ì?Èþcí*‰?Ãz9lM‰?Èþcí*‰?îzp¶ü?š™|ýHã'?¨^Ö(ô=?š™|ýHã…?çô}…Θ?µ»ê>Èîì?ÐÇôbÏ?µ»ê>Èîì3FGL J0601.0+3837@e§# –x}@"ÿŸÝÖ_À9ê+ùƒ=À;yóÐFÕ¿ÝÏàü7Q.@	9ùl?þ<ԟT±?²ût;Lm}¿än¯ñæ ¿ÆƄÜü£]¿àݺ¼$âAGNbllB2 0557+38?ïõ½ÆS¡?c­vŸKy\?T"sX¼ýÆ?c­vŸKyV?ï»\T±(?F­¯Q»?<(êÓ¶C?F­¯Q»?ïmyÑEEÙ?‰q7Œ€N§?'PÅ×WDÈ?‰q7Œ€N?ïÍÂuuP?w†VÄ >*?yÅsEWÂ?w†VÄ >,3FGL J0601.2-7036@q­••À=Ÿ½@gÏÀ82ñc…
–À;]íCdٞ?ú#«kS51@º°Í@6ß"óŽ¿Ý-¯iBA¿æ!O$Í·%¿å0Ûrµˆ¿ç®(^P'AGNfsrqPKS 0601-70?ïöƒÛØn?S—R¾‡Hö?RøIöO&"?S—R¾‡Hü?ïêõ3?o{jÚ`¿ä?eî
ÌæïÈ?o{jÚ`¿ç?îd#1њÃ?žÏVsIØè?©½ÌâæSÕ?žÏVsIØè?ïð0\,(Š?]a>PÂyò?_ŸG§®íþ?]a>PÂyø3FGL J0602.2+5314@d~`Ï6@-,}C"À9Ñêä±À;£¾:bÒ]À©ƒæTi@«¼pP±@Du߀-¸¿í'>9²ºc¿Ã¬Ò['¿Ø ÈýµLþ¿á<$§cvAGNbcuGB6 J0601+5315?ïþà¥Æq?!Xy-q?!õ£˜îXq?!Xy-q7?ïà¨Ô?{5ÿ0W?oW+€üàª?{5ÿ0Wž?ïÀšmL¤Š?{(ùžqo?²ÉY­ºp?{(ùžqu?ïÿËKÎ?š½Vñæ¥>úZsó#?š½Vñè¨3FGL J0602.8-4016@nÜ"ÿ‰;À9ó¡_`¸§À9#¾ôœõoÀ;V»ºUÑÄ?ä¾*ós«@=
¬æÓ^?þÄ6á=¿´
'½'¥½¿ÝyKyÓÍ¿Ê¿±})æ¿ã±þG÷™AGNbcuSUMSS J060251-401845?ï•aût±?…ôĨ¹‡ç?Š§"úÓ§?…ôĨ¹‡æ?ïŠl²µ*W?'ê؃ȕØ?dÓRµj[?'ê؃ȕØ?îÙ¯J.Ñ?—C@ÿvº?¢e]ò÷?—C@ÿvµ?íÖ1N¨6å?šÛû€È`?±NuŠ¾HÚ?šÛû€Èb3FGL J0603.8+2155@g"	Å!Þ?s\žà*­À9dûy‰À:þËåF@V¿þ€v²äÄ:@ɦ$Š±@βÿœ,ò¿Ý±ÙH}"£¿åö>
3¿áª<Üv°X¿ÚõÓS'pAGNbcu4C +22.12?ïþî."]?+ÿ1¹Lè,?!­Ê&?+ÿ1¹Lè]?íZb¨¸?É.zŠã;?µ,ëòº?%?É.zŠã;?ï¬>یâ?˜ƒv[
fX?œ
x$Žc®?˜ƒv[
fY?ïÿýºpØ>¸H
a‡>²/<y>0>¸H
tÎ3FGL J0604.1-4817@oö:à;>šÀ;€¦@q	XÀ:O
ª}ílÀ;¤Wèõ!€¿€‹G†¦F¬@5~ßÙïË?÷J` |!¿ï½Þÿ¦L?ïCy^]$ì?áMó½ÉÇ?˜–Œ°¹,AGNbll1ES 0602-482?ïüVLC…þ?:IÉ?R"Ÿ?=MãÐ
»?:IÉ?R"d?ïæÄÎù]?t'\wŽÑ`?iÿ;1¡ž?t'\wŽÑ^?åqg?ˆ—/µ`Ý@?Š†£¦>ø?ˆ—/µ`ÝA?ïþŽÝs³?A‡ˆõXkc?'(ÎÖæ?A‡ˆõXki3FGL J0604.7-4849@pã_€™À;€¹ Gž$À:T>iƒQÀ;ÅûqûÅß?¶Pf"ÀŽ@×_´Æq@0bŸ²bh¿á7ÈK]Ìd¿í|jŽ‹•í¿~ŒË*
j'¿é܈¬ŒeAGNbcu1RXS J060432.7-485007?ïú•Píœ?R\Ö½Áe?E«Ž¼IŽ%?R\Ö½Áe?ï¿©¯9?†º¥n"¾?€"1œŸÎ?†º¥n"¾?îôaÌ	sL?–g}¨ÛZ)? ¹ã?hËD?–g}¨ÛZ*?¯ézÈ?‰É¢Lô¥?‹RT¡MÉ?‰É¢Lô¨3FGL J0605.0+3756@eƪŽ:Á@ü.ŸûˆwÀ9³¤™_¸À;®yð'Î?û¾æ‡^@
|€È'Uƒ?ðü—x,6•?ïõ»tpüS¿ÔÙ3î"¼¿åª§Ç|¿ïp<"
œ(PSRPSRPSR J0605+3757?a8ÞXÿ#b?_l_Ä«(S?ïîÇ!§Ý?_l_Ä«(S?†µw>¿*?©º,ºâjH?六*#?©º,ºâjG?ªWsø_…? in.å/?îZˆÀz¯? in.å.ÿ?"ôALíwà?u'Ø.:`?ï¬.úÌJ ?u'Ø.:`3FGL J0606.4-4729@oܱßv½À:÷ûÀÖ…À:üLû[À;ƐY~÷W?Çû¿¥-1Î@Ë|½ë³m@žšÀ
F«¿ìœ­¹rc0¿¹"¢L×°<¿çöK¨ÂMå¿Úq84'q=AGNbcuESO 254- G 017?îeÄ-0"B?°Fd¦Ð̉?©£½,÷»Ó?°Fd¦Ð̉?îÎÔYMx?´î…Cp\&?£ºk(~'?´î…Cp\&?íDáÑn>=?§ršf2S?µØñtŽ?§ršf2U?ì¯Ð0\é¥?¬•¾LÞù?º~}²Û?¬•¾LÞù3FGL J0607.4+4739@d´xÀ>-@)ºžEÑÀ8E&s1PÀ;?uQ»´wÀ¥Ç¥EŸG@[sºÿé@.>`7ù¿äåÉkvú¿à\¬‡n/¿ßs"¦1Fc¿äª¯¶¼j)AGNbllTXS 0603+476?ïî^þô£Þ?`*:MX=­?a¡\"t?`*:MX=­?ïÝZnªø¬?}Y©Ö±?qRȪƒª?}Y©Ö­?îôé¤zp‡?—?©&p? ±e¸X÷†?—?©&p"?ïÿŒ¼&³?MÎ⟝?ÐöS9~™?MÎâŸo3FGL J0608.0-0835@jø€àe0À+>~ÀÐ?À8VÆ;¹²À;£NNA¬?äQ·
%‹@i°Ü+dˆ@û>_a9¿ÞÈc¬!Üt¿æêðü××m¿äŒñÍ'¿çŸ°·ìÏAGNfsrqPKS 0605-08?ïõ¬'èù?T˼½ê9?T¦Ü.
úø?T˼½ê9?ïÈ{'æ­µ?†"Ë‹¿u?{Âl©&?†"Ë‹¿v?î˜öÕ0Ãy?œ‡g·–ãq?¦p'¬óÈj?œ‡g·–ão?ïæï=Z[—?\¬­.g€?iÂ¥¤gÑ?\¬­.gw3FGL J0608.1-1522@kÄUŸnÅ°À0cZ _†xÀ8'™" äÀ;`l,yÏ?÷•<ÀO»Õ@O?'¡Û]@‡Xöç(¿â=³œÐæ¿ç±ë~$|¿ê±¥?s¿èKÎxژyAGNfsrqPMN J0608-1520@?ïéÞª–¨"?d>À¶N5?f!UiWn?d>À¶N7?ïªBª5ÍV?[҉€Úb?…oUrŒªr?[҉€Úb?îÔÆÛ_?•Ì¬îÅr?¢¾ž³'J?•Ì¬îÅq?îÎR£(;C?—êÞ`Æ
Ò?£ÕÍ|KÌ?—êÞ`Æ
Ò3FGL J0609.3+2131@g£? §??íÀ &jgÀ8Ӟ÷§kêÀ:Ý12I(?ýSj-E]'@
géÝSؚ?ûè!¼é*¿àñqÇÿàå»,]¿ìK¤™'¿ëz¡5¼œËPSRpsrPSR J0609+2130?Cëâ ¹?B°^"á4ˆ?ïû9~˜?B°^"á4ˆ?6r‡²žzÜ?K>[³a?ïý1¯	¬1?K>[³b?—Eíäǵ†?'1tp÷S?ïEАÙÂT?'1tp÷S?{±>¬óD?o#¬öÅö?ïÉ؝'¦?o#¬öÅö3FGL J0609.4-0248@jT&Þüz:À%AŒ 4RîÀ96ÕVß	æÀ;:"Ž½ž?Ñr†]…Iß@M>A©™?þ_O€ñ­¿àWƒ@€'{¿Ý¬)AusÓ¿ÝÙ«‰þhs¿×À›
–AGNbllNVSS J060915-024754?ïé"qø?f#GG_ÖK?flàŽï?f#GG_ÖD?ïx´±+k‹?š3ºÎ?éiڒŽ™?š3ºÎ?ïÊÅ'}\?'Iǘ'L?¦§[T°?'Iǘ'N?k?€i
³Õ¾Ö?Ž~»Pùäõ?€i
³Õ¾Ö3FGL J0610.2-2059@lwXf€À2-ПÀ$HÀ90¾£%4À;	Ü!Ôf?óûíÖ]@q-­ã(@°}_|<g¿ày·ÜBx¿âB¨ïM¿èvN—×fs¿ìŒ»[•ÄPSRPSRPSR J0610-2100?VªãìÉ(?m)Q¯¨Œ»?ïôªŽ	ø›?m)Q¯¨Œº?‰~W|Ù\?"çK)¤?
¼›?"çK)¤?¼´ø9Âü5?¬
ü~`À?ìi`øÇ z?¬
ü~`À?›2äŸb	"?†3xßäôù?ï&hÛï¶?†3xßäôù3FGL J0610.6+1728@h" ³Ô®¿èbšë±À8ÓÿgSÌ0À:ò+ÐÂü?üEy Ó4E@Êê?«ç?þ,Mìm¿ÏnA§V¿è神ç3¿ëؒ2>¿ãl¾U¼OTHERspp?Ð8Oôdµ?Ɉèp¥^Ì?çòcØͦ?Ɉèp¥^Í?šs§ð6»S?°¶Î¯C¯'?ï,bÀ~J%?°¶Î¯C¯'?ކŽ[AðÇ?»Gð>q?༸Ò_ž?»Gð>q?ªÌÙÑ9œ? ½Asäi8?îS2bïüf? ½Asäi73FGL J0611.1-6100@pá´™=SÀ<O <¶jÀ9‹€ì#ªÀ;Ó\9¼º0¿þÝ3Tk<9@ˆy½0M@£Z?¼ƒ~¿é\ºO5Œ¿æ¸Á¤>}¿é`Osä0õ¿Ú•"»T7AGNfsrqPKS 0609-609?ïÿ$w´E€?¼?Êú?q	wPù?¼?ÊA?ïêdÄ€?pn³l7
Ó?e›;óùÐ?pn³l7
Ñ?ïýñ;?;?|äx©ö¸?~!b`aô?|äx©ö±?ïÿç!2uw>ðñ™ßx>èÞ͊ˆó>ðñ™ßxp3FGL J0611.2+4323@e;R`õä@' ^YQ«À9Þî<³åÀ;¤ÏFúT?ÕL¯/æ)@´8V]°@Wé`}¿ë—&Z1ϱ¿ãn"±Ž"¿×'Œv4S‰¿Ø`|ˆAGNbcuNVSS J061107+432404?ïùïN0èS?EúaPb?HBÇ<^°Ú?EúaPb?ﷃœ­í?‡uZJíš4?'à"á?‡uZJíš4?ï¬ó$Û?ƒÝ›û,'Æ?"ý6Ü	X?ƒÝ›û,'Á?ïi_vµ(?ƒe¥G…·?'Ô?	ZÕ?ƒe¥G…¸3FGL J0611.7+2759@fõ¢Àh¡@ã:"À9«œàuöýÀ;Då1?†sðº±@.Ääv@7¹½ûN¿åÓx³£Ž™¿Ûõ>ŽŽ¬¿àÞꌃå¿îŽ'ÞQQAGNbcuGB6 J0611+2803?å¯aøT?ƪ\÷š½æ?Ô¡=èW×?ƪ\÷š½ç?ïG1äçX?©Çjiãø?žÃc.?©Çjiãø?äì*" ?¹,ºBÿ?×ãô'ª÷À?¹,ºB?îÜ2_pD½?˜Õ%œŠœ?¢<Úû´@?˜Õ%œŠ3FGL J0612.8+4122@ezWà&Eå@%Ö3À7²8%
{"À:à"Xð\?çXwýVq@@¡)3!@3å?ŠY‹¿ÙíÕǃrø¿àïr«20¿à6tJ¢¿Þ5	cÎSAGNbllB3 0609+413?ïù˜AZBÌ?Kâ¥è=?Ižú–ôÓæ?Kâ¥è@?ï€IÿïœQ?—nrÙd?í€ës?—nrÙd?ïˆÿ'»;é?Š2¼£_ê?À61ú?Š2¼£_ê'?îmÛ&L?—åhŠ7"¤?§)"M›>5?—åhŠ7"¤3FGL J0613.8-0201@jMõ¡lèÀ"—ô|ôÀ8
¤ž°ZÀ;#wÀOç@ÿ…$'@<ó%|?þ5لÁ¿¶CÛ2Qr¿ÜÜ#€Òg/¿ä°·•­ü¨¿ïJÑz kPSRPSRPSR J0613-0200?bÑF.ú?gê&/pï?ïí÷.¹ñÐ?gê&/pï?Sèæz?=	?cfiÚÇ^?ïöŒÂàa?cfiÚÇ^?¨÷¡xV÷?£×'©p5©?îp…ïHz?£×'©p5ª?W­H/ +?L¤Ð/"C?ïô9)[èq?L¤Ð/"C3FGL J0614.1-3329@nà`þG™À5Ô´ßp=€À6ì^'À:œÆä@ý#¬¦@u˜>¥­#?þÞt§Ç¯­¿À'ª~nE¿Ö…¦|X¿áXez`Í¿êz¨Ea'žPSRPSRPSR J0614-3329?'S4N±Ó^?"~y·ä*?ﶳ.Å8³?"~y·ä*?lÌýüá¤æ?vǐYY]f?ïã3[?vǐYY]f?¥5?;gô	?¢~ªaw±Ì?I€¿?¢~ªaw±Í?# ¿¯Ï$?#'õÂ\U?ïþÅôå?#'õÂ\U3FGL J0615.4-3116@mÊòŸYÌûÀ4ՙÀ0XÀ9Òâ7˜ÂÀ;ÇyÒ9À'«0ð¸º@:ÀÌäIÁ@¥@¿ ¿é_äy'¼V¿å…Â+¼¥¿á"",zåØ¿á¸]Üv…eAGNbllPKS 0613-312?ïþøt‰b?!|è%7O? x¾WiâÞ?!|è%7-?ïßy—âˆo?}$€al3?pC4»Èê?}$€al4?ïÍɡDz=?|N¥Ér?y/&â?|N¥Ép?ïÿâÜ<ôÆ>ôýSxñ>í#Ã<$Ž>ôýSxF3FGL J0617.2+5701@c­UàqÅ?@2ì_9K{À90½7-"À;"*m'ÓÒ¿úSndzÞ>@OYãÌÆ@T?b¿ÜsOa«ÛT¿ä1T>y@¿Û©NßG^õ¿ÙÛË}lg\AGNbll87GB 061258.1+570222?ïþ¢di>?#H™ï ³¬?%Ù¿9lÝ?#H™ï ³¶?ïސu‹Š?{ˆk­[_?pÀ7Å::˜?{ˆk­[_?41ë?†QÞ:>$?‡Þró¾DÐ?†QÞ:>$?ïÿ'·‡"y?o"¨‹?Rá w?o"¨`3FGL J0617.2+2234e@g¡ŠŸb0@E?ªºÔÀ5iL"=À9¯Õh|Á@M1;ŒH"@d³kýª?ûwohÁh¿ÏDô¦°ƒk¿á4U݂&¶¿áW35å?¿ä鯁7xOTHERSNRIC 443?ÀÝA/"R?ː«ˆ²2?ëȯ´ûm?ː«ˆ²3?LZ¥'ÿ›?hµ½è¶99?ïøéyÖ¶?hµ½è¶99?ÙPÝ_Β?¸ÔùN/?ãW'xж?¸ÔùN/?DŠóñ?DÄÇp@a?ïúù]`?DÄÇp@a3FGL J0617.6-1717@l¨ŸÆÚEÀ.1Ïþ°t§À92éf`‡)À;PñîÅE¿ç`Úö±!Ì@­À'U'z?þú¤¾æ°#¿ä6À'«ZP¿àb
¥^ó¿Úmœ;èí¿Ï¥{ÔP"…AGNbllCRATES J061733.67-171522.8?ïþKSB)d?'¼p·'Cd?+JËÝiÅ°?'¼p·'BÃ?ïÒÌ|¬œ?ƒ†".–0B?v™Áõ©²&?ƒ†".–0C?ïˉdâ?{éŽF+–Œ?z;MŽò}?{éŽF+–Š?ïþGh6Û?(À0^ÑÜ~?+‰|˜E©?(À0^ÑÜ*3FGL J0618.0+7819@`õÖàL'@8Üz¿¹¾ÓÀ:ZÍcˁsÀ<ÿ¼ä?娖×@Âùó÷^@ùÏãJ=¿çÖý3¿éMb˜óμ¿Ú¨O‹1U¿â/p¹"#AGNfsrq1REX J061757+7816.1?ï÷ύ÷Ë@?ZÅFTJ£?P`äi~?ZÅFTJ¬?ïw'8Bl3?™_1G[ÿ+?'
¸÷²y¬?™_1G[ÿ,?ï#S'ÛûZ?'Œ×ª{c?›•¤€"Ó?'Œ×ª{c?í±=4úÞg?¤©õeîÕ¢?²vX)Æ?¤©õeîÕ¢3FGL J0618.2-2429@lü1 žÛùÀ1Ï~¶ß%À:›¹.ŠWÀ;ÆĹØÔB?é4Ê]9tž@Ì9¶3k@U'1>¿ß¹Xôk—¿çöçMµ6¿ägÄäÝ¿ïÿ´ó‰œnAGNbcuPMN J0618-2426?î¡Å¶ß?±oâ~]S?¥ã¤'˜?±oâ~]S?Ã5ÑMkþ?Å·<˜£¯?ë2‹¬¿¥?Å·<˜£°?êsEåÑÞÆ?±ï™Žh?Æ2èh¸"é?±ï™Žh?Ì÷q¦&
?²€$]Ã?èÂ#–v|¿?²€$]Ã3FGL J0618.9-1138@ky /µÐÀ(Ø´¡\ÜzÀ9•o"'ßÀ;LžáØÀ¤ê…š^@	Ýr"rl@ÁƒÿÔa¿ç8¨¢˜h9¿åjŽ‡[˜¿çMû¹§ß‹¿ç2uâ@ AGNbcuTXS 0616-116?zñm?––°½V>?Þ!C¤˜¶?––°½V@?ï_š`Ã>?±›Éƒàž?"¼3ç˜L?±›ÉƒàŸ?íDç)ãï?¤ïÖ¸/g­?·uØÆ°à‹?¤ïÖ¸/g¬?ïý_¼Ðçú?Eû1(×?5xÀ0?Eû1(á3FGL J0620.4+2644@g6§?tŠ@‡'ŸÐ€À:F…íë*†À;ƒÜÌõ¹?Òi)ðûfy@µfEjC?úfz€NÄß¿ïÿüØ`?ïÿ›ß*ž¿×b÷ÌT×É¿àîúz¿	AGNbcuRX J0620.6+2644?ïõ5´€F0?Tݵ" ?U"–ÿsž†?Tݵ"?죮b/tS?ł8Œy/ý?ºâŒî"]f?ł8Œy/ý?ïŽÆ$!z‹?"'™-Y?ŒNv÷¡]2?"'™-U?ëOkA¥Ü?¸–Ó¨Kš?ÂÃÂRùh'?¸–Ó¨Kš3FGL J0621.0+2514@gcRàãG@;îN.ŒÀ9:ÛWªÀ;:‹#µî?ôø / V¢@6|CG}m@],¿ü"Ë?﵂·ï‰Õ¿ãèðjwµ¿Ý4À£ý¿îÜy'Š~PSRPSRPSR J0621+2514?¡)@˜la«?§w£òyÖ?îíköy9ä?§w£òyÖ?ºTKTà?Ç¢S&4€?ìµvž•~"?Ç¢S&4€?¹/²€«q?ªß·'ÒÑ?ìÚ	¯êœÑ?ªß·'ÒÐ?ÃÝ1‰÷[?¬¾H
Pêˆ?볝');?¬¾H
Pêˆ3FGL J0622.2+3747@eüãŠ	@%éW€•ÓÀ8¦'¿aª?À;…h9¥=<@4ڇöY
@èBæ.¢@Õ.=Ú¿Ó¤ÒrS.¦¿åcR§0ŸÊ¿îg
ɐ4õ¿ïþàf˜Ì{PSRPSRLAT PSR J0622+3749?ÐŚ—`þ?Ò0áÛ°?ç2´Oó?Ò0áÛ°?dV¡¸¢m?rs¦A'a?ïë©^G]"?rs¦A'a?Ë}.Täœ?²)‹›Á>?é ´jÆøX?²)‹›Á>?VÎ.,?R*{n-{?ïô˜èþù¹?R*{n-z3FGL J0622.4-2606@m:†
¢À11 ‹ü"À9u™	PâÀ;Q­nb´*¿Ý3šfž±@ T^Q?ÿÁÀTCy¿ã-¥+ëb±¿àøÐ_Ã"ï¿äª!|&—¿"/YðóXäAGNbllPMN J0622-2605?ïÿ"Ùh?"Ò
p?dÒý\g?"Ò
p?ïӓ&¿²?",»¥?v6sì &S?",»¥?ï±FDž§?'þǵðVW?ƒ®nØ|Ö\?'þǵðVX?ïÿ€'C"?¿•´bWZ?ïí׏©Y?¿•´bWì3FGL J0622.9+3326@f~¿p@"P(ßó>À7_ÿ»6¢SÀ:¾t_Mm?ñmóþ¿ä@ $¥Z—ü@¿"|üÕÔ¿ßô,.©ƒ¿äʳ¿âÑ£˜˜_¿äŘQ´ÂYAGNBCUB2 0619+33?ï÷(œ°‡î?W£ðKÓâ?Q®Æžð"Ó?W£ðKÓï?ïÏøe?Œý¾.r¢p?xxt÷ƒÌ‹?Œý¾.r¢p?îرlA?—›ä›¸±?¢té;çè?—›ä›¸±?ïÿþÄõrŸ>±®yé¯1>£°¨Ö>±®yé·ÿ3FGL J0623.3+3043@f͚€If{@ ý_çœ1À:,üۈQsÀ;«Ú
þ?ç#½É_ì@[ۓ9-H?þJ/ßÏ ¿ïÿö¡BÁ'?ïþ¨©Ú¼?Á¡í—÷'¿æ÷ãÃ÷€AGNbcuGB6 J0623+3045?ïãõo8®?q—•RÁÀi?l
ÇðSˆ?q—•RÁÀl?î	æûh"?¾û-ZOø?¯oIv»?¾û-ZOø?ï*$^Žy?'éÃøOƒ?š»t=n1?'éÃøO"?îBÑ@ýû?³†`š»?«ß¢ëð Q?³†`š»3FGL J0625.2+4440@e8OïI@,ÈFŸ ÂÀ9`+½,aÀ;'½ÝEÀÔ?–HDƒw@ºûø´\>@^È b¿älAÒæÊØ¿ãŠaçÚ"¿ÕÑéÝ­è¿Ý°6ÃOd[AGNbllGB6 J0625+4440?ïüféÜý?A¼~OˆD{?<ȱTú?A¼~OˆDh?ï×y¬6!?~Ú&ˆº—¶?tCq©äïz?~Ú&ˆº—³?ï­Œ¥Á4?…Ys/Sþ7?" ֏²?…Ys/Sþ6?ïÇJá#Nü?n,̓w?|ZnX'[?n,̓w3FGL J0626.0-5436@pu¨€QÉ÷À9ac€X€À9§Ú¥ÓdÀ;Áw=N?(?ÑÇÓÔ(
á@ã&?YÝ@]Ϡ׿ꬽo%–¿èñ2Á¸
¿åqh_åÿ¿ïþýR•gõAGNfsrqPMN J0625-5438?ïýAÌuÁ¡?;د\‹OC?5ñœQòøþ?;د\‹OW?ï)"l¯i/?¯yÌÎÎ@?šÏrjÚL?¯yÌÎÎ??ï'õ—ˆ?†›˜áª§ƒ?‹B½úÚâ?†›˜áª§‡?îeÞ§*Ê?˜LðãW•Y?©¢Wm?˜LðãW•Y3FGL J0626.6-4259@obY@x–À6hŸä6vÀ:!¾ê‹úuÀ;¥ðÍ]…?ôÁwAU
@¤f&O ?ûÖÁM½£¿æï"VZïT¿ÕËèÒ£ĿƝ_d‹è¿Óś¿}r¶AGNbcu1RXS J062635.9-425810?îƒbº–Ië?«¦4RŸ?§ÉÔV›aC?«¦4RŸ?ïªÝ™¸?—ÄK?$^?…HY'È?—ÄK?$`?鵗'¯ì?°»ðEï?É)¡¹CèJ?°»ðEð?í®'
?¨…êDžÕÃ?²‹w§¯ïä?¨…êDžÕÃ3FGL J0627.0-3529@nnƒ¡	ÐcÀ3øÄ!HÀ8ÎFªß<;À;*½•!dÕ¿ÐÓT;ý˜X@=B´Z?ýåS ¹^¿ç'chP¿ÓS0¹±<#¿ÞE]i‰þ¾¿Ø @…~bAGNrdgPKS 0625-35?ïñç5…¥?_!šÜâž]?\x±"ôµ›?_!šÜâžV?ï¾,¯®eÁ?‹8·Áªf?€tÔf´?‹8·Áªf?ïg}/g?'4µè1Nô?"ZóJ?'4µè1Nô?ïÜj]ÝÕ?jDÎo_?qÊøQ¦?jDÎod3FGL J0627.9-1517@lãø¶À(hß½jYÀ9óEî ÚkÀ;p©Ã³H—?ãÎöZS#@µú´¼Šµ@É£àDxÖ¿ãhD"œ™¿ï;Ât•dg¿Ù‡Èö?ÙÜç&•@AGNbcuNVSS J062753-152003?ïý^¡:²?<Þh?5
ö*o»?<Þh8?ïÂL°+úï?"º\ÿ϶ß?~Ù§êˆc?"º\ÿ϶Ý?ï@J´nÏd?'ÜÔ,ŽŽf?—ö©r&Š?'ÜÔ,ŽŽb?ïïÓ"'T¼?e‰7ê'~²?`,ÝØ«De?e‰7ê'~±3FGL J0629.0-6248@q{`(^ÄÀ:oc€X€À9ʉŒ\`À;ÏXK±?Íã¶ÑÁ\@ć®à~@Õ$@Q(ç¿ä}©kD,¿ãA'á2y¿âЅÛe…°¿ÔsºH!AGNbllPKS 0628-627?ïîñ´=k?k<°²k¤é?aKb"\?k<°²k¤ì?ïÏ®–AÛD?"ç™òKr%?x(´ß]Ù?"ç™òKr&?Aâ]?Šw´ÿËÿ?ŽQo‡h¹ô?Šw´ÿËü?ïJÀnóÌ¢?ŠŸÑF\"?–§ò!†kÏ?ŠŸÑF\"3FGL J0629.4-1959@l"†_•'ÍÀ+Mûþé‹À7ý0T[¡çÀ;A0Kø&?íªJ
aµ@NkåuF@u'A8¿à
øe¤A
¿äuŠFHx¿àˆM-Ê¿ä"'J¿ä)AGNbllPKS 0627-199?ïûnŽv5
?GUÍIeµ0?BEÆ'+Û?GUÍIeµR?ïÈ£=ö­?9ô)Š_?{®aq©Õ?9ô)Š_?ï#™ðšS?"§V¿à6?›ŸìÁìµ¢?"§V¿à6?ïøœ}ûrÅ?D3sB'«?MŽ4î`?D3sB'¢3FGL J0630.3+6906@b6`RP/@7b°ÿèÀ:ŒçìãÉÀ;úÌh"ÿ	¿ôßa.Ä
¶@
ÈÖ\˜‡@$ÇÛØX¿ã°»Ë·gпá´å]ÍÞ¿åR=‹7u¿êf:3Øt¡AGNbcuGB6 J0629+6900?îê…"D"?¡Îú؎²?¡^‡­Û·¸?¡Îú؎±?ïI? Ð?¤%#m¨­;?–Ø»üã?¤%#m¨­:?ì¶6º<?¨¡7º¢Ñ?ºNO2+–$?¨¡7º¢Ñ?ïÉːä¿-?|¶ÊòcÉ?{7 iê?|¶ÊòcÊ3FGL J0630.9-2406@mí_‹ÎÀ-úðþÛ<ÒÀ7ßEó)WèÀ:°3cÛW?èÚ^t™I@—v2â*'?üó'_?€ž¿ËQú"Úgë¿Þ~OñQ^¿×¾!K²¹"¿ÓNÙ|ˆ'´AGNbllTXS 0628-240?ïÓå8ƒZ?w_æ£CÿU?v
cÿ¾R®?w_æ£CÿP?ïu0Ì1ùr?˜o‹@_'?'YæyÀѯ?˜o‹@_(?îy®×õ#?¡¼{@‹ÖÖ?¨e€®=Ã?¡¼{@‹ÖÖ?îI(%54c?Ÿ&Ü_"?«m}¬¬¹Ò?Ÿ&Ü_"3FGL J0631.2+2019@hêßqêÿ@x€0¥À9fۙjZÀ;˜K»À5¿ä«—Y3´@st:9Œ¿@®èŸf7B¿åšqҚ¿éº€6œY¿á¿3]¿<°¿á¯hþ·_AGNbcuTXS 0628+203?ïýKW?;Ýh6RÔm?7S"¥PÖ?;Ýh6Rԕ?ïȎç¾d?õì"[?{¸Œ úMÚ?õì"[?îܺ¼©? 'Sè'ò?¢4T>®m? 'Sè'ð?ï÷Î:?IìÛY÷œ.?PcûÁ‹á?IìÛY÷œ/3FGL J0631.5+1036@i's`Iì³?Ýær¿~õBÀ7ö†
˚žÀ:ÙҢϣA@– ´Ö`õ@
ý6E'@?õ8{Çw¿ÕF
ë_¿Ý.×výk¿âžržzv`¿ìO^\#8âPSRPSRPSR J0631+1036?Dô@@ØwU?9DÒYxéW?ïúÂïïÉâ?9DÒYxéX?3f'?K•í™ä?ïýž3?}¾?K•í™ä?€ùT`Á?|$(%F]]?ï¼®}øû?|$(%F]S?nÎÏû?µ?a)«r—(p?ïá~10À?a)«r—(p3FGL J0631.6+0644@i•¥¿­)™¿ôàÖ¿"ÕåÀ8"^ëGâÀ:–½öp4F?ù‡ÉûŒ'ì@ø'÷ŽÂ?÷­TF©1½¿—Õž'ŒŒÁ¿âà"~¿á7ɀ2W¿ìŒ˜_ö"OTHERspp?7¢¢E2dé?2?«¯mb™?ïý«·Y³?2?«¯mb˜?STàYS÷?j}´×	%?ïöUÓ{Ö?j}´×	$?'/›ö?7	IÇ@	?ïnƒ'ï¸O?7	IÇ@?Ÿ­Ld¶¹›?Ç#;•;Õ?ï•œÚJ3?Ç#;•;Ö3FGL J0633.7+0632@i£¿YFÿí»8 
•
À6ιƒCì¿À:Z֒Hl€@Ï)à#@Í@Vð9Žl@Ãë&Õù¿ÒSŽ:žj¿á0<<‹'¿æ9vTH¿í~Žè ÷PSRPSRLAT PSR J0633+0632?BN{˜ƒ@?9þÕH.?ïûlaß1?9þÕH.?#m¯ÏÖ¦?D'Y'tW?ïþÉ%ž?D'Y'tW?tBÙoc?Y/"ÿN¾?ï×zM á9?Y/"ÿNÎ?+·ÚîÈé}?&r®;éÿ°?ïþD'Qp?&r®;éÿ¯3FGL J0633.9+1746@hdA¿½ð'@'H$\À3L­áO:ÑÀ9=XJ@Äòýãñ@¶¥¹7™Ÿ?ôP'Ldë¿ÀŠ(æ¿ÚeR˜[߂¿ååðy+¿îA÷~§$òPSRPSRPSR J0633+1746?'$‡ÁHA?!Èјö¡?ïþ­·ƒê?!Èјö¡?ONÁ1%W3?r*Nb?ïø,O³¶«?r*Nb?uI'õ®n?nB+&æS?ïÕlúà¢?nB+&æG>e§¾¬x]k>t‹ˆ
`fÀ?ïÿÿêXAT>t‹ˆ
`fÀ3FGL J0634.7-2334@mû 1ίÀ+ýüߺ[À9£€)†À;ëˆy¶¥?欠tª û@?s­KÓ@JE Eš¿¿çm!W­TÑ¿åò¢ô@ã¿ëäTc ÿïÿL]?ýAGNfsrqPMN J0634-2335?ﮍÞ|_ì?Š†úÛOým?"\ˆ`è?Š†úÛOýn?å«[9jí?Ðþn®˜P"?Ô©ÝI*'?Ðþn®˜P"?ìíRÈ~9?§ÒEɋ#??¸•i¼;?§ÒEɋ#=?â倈jÂ`?ºñ
à…?Ú4þï*{??ºñ
à…3FGL J0635.7-7517@qæG rѯÀ;)_JsÀ86
ÄÀ;•« éð?æÅ]‰ÀU@eºsY@®àI+m¿æ¶{v1ÏJ¿è]¦öh@u¿ë,͑Ôå[¿ïÿ.¶÷£eAGNfsrqPKS 0637-75?ïù§ùû!P?Kì0/OÀ?I`zÀ1?Kì0/OÍ?ïã?è¯p©?v©*ø;%?lÀPWg?v©*ø;&?ïKfºV_@?ØÞ'?–"(µ4Ö?ØÞ"?ïç§H•0™?cJŠ¯?hX·jÏg ?cJŠ¯3FGL J0638.6+7324@a¨ Àiçû@9¬OkxÀ9—}K…9À;ÝM×#gä¿Ñ{Ë6Žv?@.²§²Œ@笳¿æS<ã¹á¿éj;ÿE׿ä=š?\¿ïÿ©ü=RÇAGNfsrqS5 0633+73?ïÿì±µ‹>ò¯Ø>ãNJbv	á>ò¯
U?ïÎ@Xq¬K?€ÂkÓc¸¹?xßÓÇ)Ú@?€ÂkÓc¸º?ï¹ £ªp?cżƒ­?¸××d?cżƒ¯?ïììC§'?^ëë–KÜ?cä¼X|ç?^ëë–KØ3FGL J0640.0-1252@kæHÿ¸²dÀ ŸóI"À9æ´5&RÀ;UHf¡?à9¶{#@
ÔÍLN?ø3@¿bÖå?ïò>Çøþ¿àV³üyì3?Ëò«{ã¿ÌŸÀÿRõµAGNbcuTXS 0637-128?ïÝèÒ&rg?s²÷PðH?q–ìÆË8?s²÷PðF?ïJâ;T:?¦VçáÝô?–£¸•~°?¦VçáÝô?ïsÛñ?''î¿rç‡?žñÄœí?''î¿rç†?ïÙ扵c¸?uúêôUîå?s»%N$-?uúêôUîè3FGL J0640.9+0752@i—]÷vÅ?ô}^?{kÀ9Ï!j´À:Í"4H?¸Vº£‰ÅW@
]lŽôz@rZ¿i6û¿äu§L
¿êÂ]B¡¿ê)^ž	¿ÑÒã|¼"OTHERspp?å¹5BHt›?ÏtÊÒ³?ԍ•{oË?ÏtÊÒ´?å¥Å~i9è?Ô\Õ;£=Ä?Ô´u-Œ/?Ô\Õ;£=Å?çÔrÓëf?ºeN"M+?ÐWÐX)3?ºeN"M+?íóŸ'Q
ƒ?¥ŠÝ#
´‰?°cmw"á?¥ŠÝ#
´‰3FGL J0641.8-0319@jÙ¦ %9uÀ
gßbP­À9‡86¨2ºÀ;¯#nš?çÞKpåW@¬¡ÚZÔã@¢Êi²K¿æZ×ä⣿ã=*É(å¿ãÀãîZÙ¿ïÿôG÷ ÅAGNbcuTXS 0639-032?ï⢩W?"ÞfSnTà?mì]æV¨Ø?"ÞfSnTÞ?íÞ©Qø?ºž0]X/?±
µp?T?ºž0]X/?ëf"r?©¡+©d¼»?Á¿¾dõî8?©¡+©d¼»?ïšµôõ#?'(–.Ùã'?©Aa[˜?'(–.Ùã'3FGL J0643.2+0859@i®ÀrKw@:ßkàÏÀ8dbzÀ:ÎÜq…~?ùûdg@Ú3më–@ÜN®¹¼O¿Þÿi;Ö¿ä»`ã¼õ·¿è|s±±¿ïÿ…"
ì'AGNfsrqPMN J0643+0857?ízw½yQ?µlÎú¿+?´,B5w¥?µlÎú¿+?ç«¡ÍÒ¸‡?Ñò­mÃ?Ш¼dZŽñ?Ñò­mÃ?æóŸoÏ?µNђ¶L?ÓÄÁ b?µNђ¶K?çãÅêhMl?¸!MÆi??Ð8t+/e'?¸!MÆi?3FGL J0643.4-5358@pu3?ÈlìÀ6ÆfÙ×À:
Oa´À;Ç1Xg "¿òó—Œy§@Ùê†7"@Œy¦Žu¿êN=ÄAôþ¿×%ƒˆÇJ"¿ç½z_þ©z¿èñ04;AGNbcuPMN J0643-5358?ïàiöŠ?s{À²,¾b?o–ðé	uó?s{À²,¾_?ïä"ÃÜe?x.'½?kÝ<#ïšV?x.'½?#'1Z?š`hÁT?¦FM͌ê_?š`hÁQ?ïü÷£ï6í?6Ö¡±ö
=?8Bà†H–I?6Ö¡±ö
G3FGL J0644.3-6713@qX—ÿ›V2À9‰4ŸCý†À7ØýCŠÀ;åÉä?ìD™ùw@Ou¬ªm|@ÂÿýfH¿àý'²Ìq¿áæ
n £¿à½ëtœxá¿åS
æ&ÔÅAGNbcuPKS 0644-671?ïþ#a]F?1‰'igð©?-Éê&+"£?1‰'igð?ïèCA{ëM?s명/M?g¼¾"±m?s명/M?ï|KqAû§?Sà"A&?v'×À‹?Sà"A#?ïÿ
;û±?Ë/Û¸Jü?X‰Í"?Ë/Û¸K3FGL J0644.6-2853@mÏ:ÿ°NèÀ,.z WŽ\À:_Ï2ÚÌÀ;Ä}‹F¿×{ٌ›%Ø@d‹šÓU}@㦿qð]¿ït¾§VVà?å	k©qRþ¿Üù»ŠA¸¿ëP"T'±AGNbcu1RXS J064444.2-285120?ïˆoQÛ£:?'!H®íjý?ä+‰1†?'!H®íjý?ïDÑ»\Ê?¥1CÈ%w?—eÝ("f•?¥1CÈ%w?ë͏ým?®†g¼C"?ÀËÁü
J?®†g¼C"?ï˹ýŽÀ?x¸£Nìî¢?z#u8 c?x¸£NìîŸ3FGL J0645.9-3914@o@ßXÀ‹À1À¶àÒ=OÀ:ª>,‹À;Á¦V]ÛÀõ‹¾åƒ}@Ê'D½t@'ù gÔ{¿êI»üke¿é
šO±™¿å«¤¶£¸¿ïÿ1¾¾íAGNfsrqPKS 0644-390?ïùՀ§,ö?OÓ"i?H©ýcL&à?OÓ"c?ïл>Z_'?…êÖM¼ik?w¢`ÒÐ6ä?…êÖM¼ik?ïÕid­7?¨<Ð*i?œåRÓjY?¨<Ð*k?ïÿ‡/¼>?*ê"#?4ÿpËX?*ê"ç3FGL J0646.4-5452@p†Z\FRÀ6˜À§¨À:±Œ7±G5À<w&0ì1?öaÖâOj÷@!VØÿ¶¿È]¢Pþ?ï¯ù͋äz¿ÚՕŽ7ï¿èÛ~re'ï¿ïþÞdFHAGNbcuPMN J0646-5451?Æ…F?ÕXÙSÚÔ_?êz¸ÿx¯?ÕXÙSÚÔ_?£œ-—+ò?Á ýâpR?îÆ=.vA?Á ýâpR?Äß!ái?±ƒåÄt¾°?êÈ7‡¼9æ?±ƒåÄt¾°?µrh§?·; À™ê?í^®Rþ
?·; À™ë3FGL J0647.0-5134@pOø!ïÀ5"Ð_ÿDÀ:C*È*§À;ڈ§ÙÎ=?Å$ÿÇSš@
âÖ¤fý@ƒâ?Ð¥t¿çÈÓ*^¿æb5a¶©J¿Ø–8¥³%¿ÑyFðKÏYAGNbcu1ES 0646-515?ïù<.ÈH"?Scå±ÀÍ?KDÞßpò?Scå±ÀÊ?ﻊº¤sË?¨|c=?QVã
?¨|c;?ïœø$Éx?"ÝÇxóT?ˆÁöÿ¢?"ÝÇxóZ?ï'àY·ª?"®¹2ǎ#?Gúi'm?"®¹2ǎ#3FGL J0647.1-4415@o²Í ¯¢ðÀ3I`ÆuÀ:œç+ó¤À;ÙLhÏÍ?¼ýaÄYûc@]†ÎÇ8@Ás\f³¿ìôyI˃ª¿åÐhYíî?Æ ?ïìÒRzÌ$AGNbcuSUMSS J064648-441929?îâé&zn?ºPp‡tÐ?®ÑÑm˜Y+?ºPp‡tÐ?î^V"¦r?»F•`?ª–Æ%˜Ð?»F•`?ìù"þ†(?­´>·hÛ=?¸3ػβ?­´>·hÛ;?ï&JyîŸ?¥Ôâ+A?›6°Â,ý?¥Ôâ+@3FGL J0647.6-6058@píοìºÀ7ñàè@À9KTÛúg:À;­ÈŽyªç¿'t8w÷@ŸŠùB̃@±¡ y1ſޟÜaÈÐq¿åd'ït¿ä3Æ£_c¿ç,=¾&–ÃAGNbcuPMN J0647-6058?ïø¸uœ·a?‰ËÃÄ0&?M)"~?‰ËÃÄ0(?ïÑöòov?€÷.r?áä?w†È1Dã?€÷.r?áä?ï€õÊ,V7?‰^·ˆÅ3Z?Âtêr?‰^·ˆÅ3T?ïËMù9^S?oFvì=¹w?zYcPÕÅ?oFvì=¹u3FGL J0648.1+1606@hÅZÀ?ö@A.Àë­À:…Ç7bÀ;±'[¶¿ížðÆ|&@SöâŸòÏ?üdÞßHûG¿ë\Šfd§¹¿æ̶Êàl¿ØHZ¾"Ì¿ÝOŽéðÓAGNbcu1RXS J064814.1+160708?ïþ«('—]?)ç,'Ý"?%MvæŠ(ƒ?)ç,'Ý,?ïÁèÞîÜ{?'{#Q²K?ˆ'Ã?'{#Q²J?ïÃæ"K¼?xò̤|Ð?~s¶Z!w?xò̤|Í?ïòŒ~Jå?^Ó4`²?ZçÕj4{?^Ó4`§3FGL J0648.1-3045@nÈ˒:À,BIÿ''ìÀ8áfãcèÀ;rÍ 1cO¿¼Ü+Ë­4@GÜ7£Û@te€¿æ#­5F¢–¿èZçï+á¿ãHþ®òf¿è»zóoAGNfsrqPKS 0646-306?ïÿe·®Gå?Âvb™?I
7\Ï?Âvbˆ?ïÝÐq?‹Èñd?qrqu—Ç%?‹Èñe?ïÒurH´?y|ÚVî¹?vÅFÛ¥öP?y|ÚVîÄ?ïÿå9K"¥>ë>ÎP0Ì>êÆ´lZ¢´>ë>ÎP0ËF3FGL J0648.8+1516@hߚŸ¾vÉ@VÚ`SaÀ8ÄN¨¿¨À;ÚaàŨ¿èÞn3ÔÂ@­@͵€?ýKF(_?ÍF:™Pjô¿Ôl.[ ü¿¿×``¹Û¿Ù-Á¼î‹AGNbllRX J0648.7+1516?ï¦å—~ôQ?ŽXí—Mý?†Fš Bë¯?ŽXí—N?ï€È?žÚ[€±C?üûÍú¹Š?žÚ[€±C?NFî?›'µG€x?¦WK÷?›'µG€xš?ïËDZ²Ü?w"ö‰Û¾Œ?z'&'öÎ?w"ö‰Û¾Ž3FGL J0648.8-1740@lŒ`Ëò²À!9ÿÖ•À9aéÐé'ÿÀ;%HŽå?Éoà<+ø@¾ß"	v@(Mß[ð—¿è`.'ô¿ãÉç'/y¿éѼø»¿åº4!xSAGNfsrqTXS 0646-176?ïðÙ³åCD?fœæáL?^L˜5yx'?fœæáL?ï^¦«;î?¥ÿ*ŸwÝ?"+-ꘂ ?¥ÿ*ŸwÝ?îø«¿m'·?"£²ÿ¤F? uD	-"œ?"£²ÿ¤G?ïòùFF´?R6‡»ÙU?Zßsr™‡?R6‡»Ùa3FGL J0649.6-3138@n06¿DNÀ,d:a$ÞÀ9¬þ›{ñéÀ;`œ
è ?ͯzVˆLë@¸±¤þ&·?û¨² yL¿ìýkÆLªþ?Þý*ÍŽØ¿Ãsýyy#é¿Û­fѬk¿AGNbcu1RXS J064933.8-313914?ïâB³Bˆ?q¡"Ðk§?m½Lç½w×?q¡"Ðk§?豈>å?–¶ðÄÖa?†ßð}à?–¶ðÄÖa!?ï…ã³H˜¶?†]v5O»ß?Ž‡-ÙÒ`?†]v5O»á?ï‹â}Ž,ì?‡¸	@«ÇÏ?`œtÄà?‡¸	@«ÇÎ3FGL J0650.4-1636@lv²gÇÀÓþ_ìÏ¢À9.Wø™÷À;Æ폺ô?ðûc"xB\@håòŽ@uâÿi,>¿ÚéÒU'›¸¿æ[xt
¿é€îIõ˜¿ç¯£2ìÞ²AGNbcuPKS 0648-16?áëÐ_±?΄§F-Ÿ›?Ýà(_@û?΄§F-Ÿ›?âå´%\ô?Ôµ'L¦´?Ú4—µGè?Ôµ'L¦´?âíè²98ª?¹Z8'þ'"?Ú$.›Ž¬?¹Z8'þ'"?ÛúlŒn]?³ 9<á?âɹÈÑt?³ 9<á3FGL J0650.5+2055@hA}`éNä@"c.Àë­À9¶'Ã]À;Th®?C¿°[5ÑÎ2`@«–ÌŠ²¡?ø@W¿ê»b‹TKK¿ØêpY·ßÞ?›FAi#¿Âôû#ÞAGNbcu1RXS J065033.9+205603?ïø,5­?HW‡:ìCµ?OóO)K¶B?HW‡:ìC²?ïѾí
?‡P5"ê?w ý‰y?@?‡P5"ê?ïg7vd¼?…–®¾"Ö?ˆ¦2"fÐù?…–®¾"Ù?ïú$ £"÷?DËéÑN•ï?Go}q¬&ß?DËéÑN–3FGL J0650.7+2503@gȱ ‹ü"@&ðál—À8F-ù7ŽãÀ:мž_ç¿ÞÂrYzH@ 9#¸?ûˆ~žìiË¿Ób"ý[>¿ÜυÜé-¿Ð¦=Y°S"¿Ôà©3¦²AGNbll1ES 0647+250?ï÷{I=†?P"*	ÑÃ?Q	m݄óš?P"*	ÑÖ?ïÛc™¦Ú?|o¸D&kß?rNq³,'‡?|o¸D&kÞ?ï¤öÕ­@›?‡`ÑWö~'?†ÂJ"¯Ù.?‡`ÑWö~"?ïö¹œ2r?S°†2µ;?RŒÇ›Õî?S°†2µ;3FGL J0651.3+4014@eýÓX"@1­ _À:«õ¼°À;ËÌ%ÝàÀlæ.D@ø{
bZ@õþ€y0¿ÕOÌÔâùh¿éùIЃ'¿Åš—ùäæ¿Ünf¶©†AGNbcuRX J0651.0+4013?ïÿ¶e†å¬?%G·¥›k?fžF•u?%G·¥›Ž?ïæ¯Tõ[U?u7R[AÑ?iP«
¤«L?u7R[AÒ?ïË	òL«´?yqÈeß?z{Ùª&?yqÈeÞ?ïÿþÔ¢2>²ÞÁ\³ò*>¢µÞ|Ò©	>²ÞÁ\³Ë3FGL J0652.0-4808@pQ?´‰À3ÀÆ3¡îÀ:iñxôÀ;×PÁ¹sT?êº°‰íw@
üxŒØ@Z"`Ÿ§ü¿ëœ†ÀŠ/¿æf1ýþóæ¿ÝBÛB—f?œ^yæ~'EAGNbcu1RXS J065201.0-480858?ïðÒ}NûZ?f¹e³e?^[b	J?f¹e³b?ﻫ*úèí?Š/vgm€?5AEÄÃ?Š/vgm"?î¨uKø"?›Ï>J4?¥~(«@w¾?›Ï>J3?îöf/–z?ÉD¯O? ŸÉ˜V?ÉD¯O	3FGL J0653.6+2817@gqXf€@)Ú'ÿ"ŠoÀ9£/…(ÉÀ;¶ÄnYyï¿þK_§…jŽ@èžd"@ÿâ'…¤¿è\Žab'¿ã55¬E¿ÐuÛӔ«ã¿éå¡9ËþœAGNbcuGB6 J0653+2816?ïêCÖËq«?g?¸E:ŽY?e¼)4ŽUC?g?¸E:Ž_?ïã%h×z"?xÂó°=ªñ?lڗ(…mH?xÂó°=ªñ?î#JÊ?¢ÀvZ:C?­Îß~»Sd?¢ÀvZ:C?ïÿ'åÆü?ïó»(Z?{†ŽA
v?ïó»(è3FGL J0654.4+4514@efŠá'6@3cS`Ð$pÀ8ºp©¶À;Vä'Ë÷»?ì²*3Uö@Vn=Í@L_ß¹Ž'¿á#±¿å0ŸZ"á¿ã[ù¥óÅ	¿æ¶ÿNAGNFSRQB3 0650+453?ïþêÕͧ?ô€eh?!R£%ŽÜ"?ô€eÙ?ïÛ©U5?|ñ04M–È?r+Uzepó?|ñ04M–É?ï|H~,U?ŠGœZÝ5?vð:uMÅ?ŠGœZÝ7?ïÿç^yµí>î(,œ¬ký>衆JuV>î(,œ¬co3FGL J0654.4+5042@d¶êá‹@5w ÈÍdÀ8Þˆò'À;y\*£A¹?öŒ¬KMl@<³µ¥?ü¢õ°pÌ¿Õj=p£×
¿àËp¶÷M¿âmX•dοæþŽÆÚ
AGNfsrqGB6 J0654+5042?ïðêÄé	Z?`?¥'±™?^*v-íMÊ?`?¥'±™?ïÎ_Ø?Òd?'éíâ.R?xÐàÍÎ?'éíâ.S?íÒK!çW¯?¡ÉŠ42à?±m¦ðÅBƒ?¡ÉŠ42ß?ï~°£`Ã?"]øó[Ž?)ë"ýdž?"]øó[3FGL J0654.5+0926@i›``þG™@é‹@•À9ÁÃèø|~À;]²_c<æ?ÔS~"|ñ@þP
.'@S©"Ð\¿à"Câ¶v¨¿ê-ûL&¿êÝQõk&•¿ïÿcÚ½GÁAGNbcuRX J0654.3+0925?ï]'&Šµw?¡G¤!å?"MÛ.©Q/?¡G¤!å?éÞÁeKžn?Í3Bö'˜?ȄújцG?Í3Bö'˜?ìrgË%/`?¦µŸ9"ÖŸ?¼lÁ¦Ö…?¦µŸ9"ÖŸ?å1¥Þ´ p?¹ñÅûiòš?՜´B–¿"?¹ñÅûiòš3FGL J0656.2-0323@kÊ¿ÞñßÆ£'À8NAûMØÀ:Óïµ/!V?ûÇwB¬¢á@ö{ÐÛÐ@lj
µ¼¿Þ…!vŒ6¿æÔ<k§T)¿åQÇ™8e¿í²ðF"QAGNfsrqTXS 0653-033?íiPßS\?²Tg­8h…?´µ1e?²Tg­8h…?ÛCBe:âX?×<"‹)¤¾?â^^ÍbŽÔ?×<"‹)¤¾?ékšTØÐT?°â•8?ÊQ–¬œ¾±?°â•8?è*RK¸ò•?·ÿÛ¢O?ÏV¶Ñ5«?·ÿÛ¢O3FGL J0656.4+4232@eÀâ€'،@2жâ—À9¤ÛÍÐfÀ;Ÿ<zڑ±¿¨›æûÍr@=¹±¼ûô@œ3`ª¶¿áÔÒKfÜ¿èäbÉ+‹¿Éß´à5Ï	¿äúµÝ`ÝAGNbll4C +42.22?ïëúwYSV?"—YªZ³³?dˆ¦¬©r?"—YªZ³´?ï§õu2?ŽaÂÝ*Q?†¼xâ³`?ŽaÂÝ*P?ï®\~âA?'ëž2M­9?"hàyof?'ëž2M­4?ïvç5»X?‡W\ϋT?'#ùH"ì?‡W\ϋT3FGL J0658.3-5832@pË¿ƒ8.À6…rÀ:cþtŖÀ;×~ßÙïË¿ûa
Œ±@`Ï«¤^@7(`Ff¿ëM:£óm¿ÎK6Ù ¿ë÷"Èú&Å¿Ô;aSñ³{AGNbcuPMN J0658-5840?ï|Ñ+ù¾?'¤0ý:4?|ڀÈ)?'¤0ý:4?ïå">Ù='?v>dق½_?jÝÁ&Âmv?v>dق½_?íà•b8ø? {¥´	Ž"?°ûTî8?û? {¥´	Ž—?ïýÆ+Sä?=Þ±&]=?7¹Î¥`à1?=Þ±&]=&3FGL J0658.6+0636@iûg_ö	Ý@_ú D®†À9¤Ï©öÞïÀ;Y#)гâ¿ÝËY'¡@ãA¯¢Åg@ØeêV ¿èí¯½¿¶¿âî`<Î	¿çq¥õ¢"¿Ý'ô)¢AGNbcuNVSS J065844+063711?ï¶øÀº¥²?ƒP{eI?'AÏÑV"y?ƒP{eJ?ï•T»Â_²?˜#iÕÃp?ŠªÑh<?˜#iÕÃp?íÞ`ódË?žš´ý>»Ê?±øgÔٙ?žš´ý>»Í?ï˜e?¾?¾›ÖÕʹ?‰æ»°:±?¾›ÖÕʹ3FGL J0659.5+1414@i"‰€²B@ oNó[À8I?>Ú0cÀ;_ÆÞ?ÿä+mìí@ëäj"^@
ùٕˆ¿äÛUiú¿ìZi}že¿ì­Tcuv¿ï5IçÙ"PSRPSRPSR J0659+1414?˜­6mû?¿§RÛU»o?ëYûT²d'?¿§RÛU»p?±tINßH@?Ç	ûëù<?íÑvÖ$÷?Ç	ûëù<?Þp¨ž
ÿã?´Ø)!êR?àÇ«°ú€?´Ø)!êR?sgêhá?€ç¢áNF$?ïÙû0+Ã-?€ç¢áNF$3FGL J0700.0+1709@hÏ_¿ƒ8.@#. ÿê[~À9O7¢KðÀ;}x–ê'°?îÕÇOèÔ@8Ej˜O@Ÿ 䨿刻®tü¿ê"m/¥¬¿å
îޚž¿ïÿœ¹šÒAGNbcuTXS 0657+172?î pN\h?®&îœz&?¥øû9€?®&îœz&?à¥ÒX·m?Фv'
½U?ßâ´[N''?Фv'
½U?êÁ}1gf?±ü}ã$«p?Çüú:be?±ü}ã$«o?Õ¨ÞÜm_?´Á?Æ…?å+ó'ÉO?´Á?Æ…3FGL J0700.2+1304@iFÜ¿ôw6@kóæAÀ:6±n¢u
À;œÃT~–?ù?å{Íß@Bs`õ¹*?üഀz¹°¿ïÿ¦´	\u?ïþî j¿Î¿âhµw+ì©¿Ü2qÞrDAGNbcuGB6 J0700+1304?ïùXžëæ'?Iû|d©/7?J"Pe»•?Iû|d©/"?ìûdž?Ä/¨¤t"À?¸'	ÃËú?Ä/¨¤t"À?µ 'Š?€'uÊq?ˆR—öÜ?€'uÊq?ëw÷‡X?¶ ¿ôÜè? !㾟š?¶ ¿ôÜç3FGL J0700.3-6310@q`4óþÀ7	õ`iÍ#À:nߋrÀ;é}ü…!?ÖIÀ'*€÷@pL'8?ÿåÎÿ'r¿ìÃû"­Ãê¿ÎOÀêb×2¿Ô@¿©´Õñ¿çb=üAGNbcuSUMSS J065958-631238?ïö$}¥ÄI?_HƒÒà"Õ?S·´wod?_HƒÒà"×?ïś')ã£?…°sÍ:f?}2lk-Ì?…°sÍ:f?ï'ð=y,a?ˆE皮k?‹ƒð¡´çÄ?ˆE皮i?çüˆ;?€í\èàÊt?\FÝñ°?€í\èàÊt3FGL J0700.6-6610@qL>_·¼À7¿F uÁMÀ8Á¯bYÀ;"–ÇWB?òâz뮏@ìéÄTXG@ˆì |··¿×zFm!Áq¿â.ƒç^Q"¿áˆYeµ¿åôbèØqAGNbllPKS 0700-661?ïú†5–Ã1?L•Ð1Lç©?Eç)¤ó5¨?L•Ð1Lç–?ï0ý—JYÚ?¢¬H?m?™àM´Ä›?¢¬H?m?q|³?Â¨žŽ3"?§7Èè4Ή?Â¨žŽ3'?ìf"Jj¶è?¬ÑY^ӕ×?¼ËݬªHÆ?¬ÑY^ӕ×3FGL J0701.4-4634@p®ŸðË°À1»yß¿î˜À8®àŸ°4À;aš>G?ö—b˜ì@wëb<á@''afÍ?¿âDuÖ¤o"¿äH†¿éuE£'¿¿ïÿ‹TÌ#ôAGNfsrqPKS 0700-465?ï£?BX´?‡´â‰ÉI%?‡0/})ÓC?‡´â‰ÉI&?ïÄõ‰Ëç'?‹àýè4[º?}…;kò?‹àýè4[»?êZõIçÞ?®Û»\\&Ò?Ɣ*Ø`‡É?®Û»\\&Ô?ïØNë%?p¡ÛG"µ	?sÿ؊m~S?p¡ÛG"µ3FGL J0702.7-1952@lþ"Àh¡À#j ñÀ9aLF)¯ýÀ;Cä6uÝÓ?ÔcÍ,̚V@…©Îðéb@€ã?ëÓ¿å°p#¿ÐBÜtœ¿à~8iE`¿çb,žª¶´AGNbllTXS 0700-197?ïÓÊ\¨?sPqù^H?vÑô«ÿx?sPqù^D?î3Ü©­?·c§Iœr?®¬Â5oE??·c§Iœr?р
ñ?›!utÁ&-?¤5Bçÿ Þ?›!utÁ&.?ïëZËÚ?ˆÕ¿-¡ ?œ¿¢"¦"­?ˆÕ¿-¡ 3FGL J0703.4-3914@o;¶m
JÀ-;@Î&iÀ9›Wò/\åÀ;˜ôs®N?ð¹$y\@hó
¤×@M®€0'î¿Þqèa¿äphÈÁ¿ä­™<Ý¿êÂx‹%AGNbcu1RXS J070312.7-391417?庼"'2f?ʹÎ
tz?Ԋ†÷±›5?ʹÎ
tz?ê˜Í>õ¥?Æb"—¹*?ŜËð)m?Æb"—¹*?àxn‡or?¿G_@rŠ?ß"Äñ!?¿G_@rˆ?äv ƒXéG?¬õM™á?×¾ùN-q?¬õM™á3FGL J0706.1-4849@p4Ó_ôöÀ1ËóÀVœÅÀ9ob–PÀ;rd­(—?¨	,eÃç@qHA¸1@K¹ÆÄË¿Ý°¨vM±†¿çÖ?#P'¿ä¡‹^ $k¿çzÌìF(AGNbcuPMN J0705-4847?ï…S_9Dy?'e—°ô®p?Ž«(1®áp?'e—°ô®p?ïq` ¯.ñ?™M"ÄDã1?'Óûê!Ó?™M"ÄDã1?íU¬‰'ãY?¦>.3ês?µR›³på+?¦>.3ês?îüŒ8 F/?‹/;iÍ»æ? 7<}ûœé?‹/;iÍ»æ3FGL J0706.5+3744@fo•_x5œ@2ý¾?kOÚÀ9ºgozâÀ;Zˆ
%ð¿òےîÔ @ùó×'ĕ?þ= }Îã¿Øü½¦û=4¿ß£îX_¿àc§wÜ8¿Ñ-3FuҌAGNbllGB6 J0706+3744?ïÁƶ›…c?³r°ç"!?¤²=N'?³r°ç""?ïÙó¦i¬
?|¨ªsÁ†k?s,Ë)ù?|¨ªsÁ†l?ïô²d';?"wP6tÀx?ži³o¸™?"wP6tÀz?ïúÉõ?JŒ›~¦uS?GäÛëð*z?JŒ›~¦u]3FGL J0707.0+7741@a¦°)(@;H¡€èTÀ8監À;—³%]?èð¬Q}l@ø×è3Û@k_\1¿àd€Ý't¿ß÷ÿ`GéN¿ÞÎö ˆ¿åÆ9¤€AAGNbllNVSS J070651+774137?ïýˆÎ€H?4¿ná>:J?7¹‹ýÆ,?4¿ná>:q?ïÄô"¶ËI?ƒ%å
Z¢?}…½¤š\l?ƒ%å
Z¢?ï£$¨D¦£?^Ék ÈÒ?‡6ÕîÖWN?^Ék È×?ï·g®9·?rۆ.cû?'&:Tq':?rۆ.cû3FGL J0707.2+6101@chy?ò^W@9a°,XÀ:aÆÄuÀ;ú'ÌÍ£Œ¿Ü+¹†ã­@`B_A@o Ÿ1ß¿çH©`['¿êB;ԗqv¿áEC#XØ¿ïÿ¤TÕç AGNbllTXS 0702+612?ïþ‡UD¤Ú?2
._ë}]?'Š«µ²_?2
._ë}?ï—£ED8?£½«/æ³t?—Wy#?£½«/æ³t?ïf¢é"y?‹é
9ç <?"+¢Íæ?‹é
9ç <?ïm=ù?ŠsM>;
ð?'X@Â(*›?ŠsM>;
ñ3FGL J0708.9+2239@hHtÿ†]}@+•³rì‡À9ñÅíhNÀ;²$€€Ä?áo'èƒP@$Êû¼Nz@œ¬_nû`¿"C2jòxi¿à'–6Hø~¿Üa=Yt1ø¿éR6u Ø,AGNbcuGB6 J0708+2241?ï
ÅQÝý?¡TŽ;
v[?žG_uÄ@]?¡TŽ;
v[?ï}Uø––?"W^vÿã5?U_€í-)?"W^vÿã7?ì__")?¯L6Ù·Ä?½õ^·ê?¯L6Ù·Ã?î-$
!"E?"Ÿ`}´×â?­-¿]滲?"Ÿ`}´×â3FGL J0709.7-0256@k4œÆø@ß
ÿÇöÏÀ8JoÛZ.JÀ;³¦‹¤?ÜM$ñ|²@õ(‹k@‰û Iáö¿àÌTw%¦X¿çŒðw]ê¿á5pËL͗¿ç+óÀÎßAGNbllPMN J0709-0255?ïüç_$>"?BיRË?8ÅÞ`0?BיRË?渚ârÈÃ?"š'v+}k?…žGcMÏ\?"š'v+}k?ï17àÖæ?"öúÃÊ{?™Ùå#S?"öúÃÊ{"?ïú;åo´‡?AFŠ"·—?GjA-á»?AFŠ"·|3FGL J0710.3+5908@c¬|àü.º@9h~_o×À9ržJßÀ;ljÌ&´ ?Àæºòã?‰@ŽfÇ4?ú"—!U<¿ãÌÂó	¿Þ1ãAÙ>J¿ØK«"ÛÙI¿"r¦›N"AGNbll1H 0658+595?ï÷K;'Q?Q·ŒÔˆ5?QiˆÛß^<?Q·ŒÔˆ-?ïÖÅð›
]?~A˪7ØT?t²zÑ3?~A˪7ØS?ïŽBa1É^?‡°F=q3?Œog³¨`?‡°F=q5?ïïž={æ?Ww">8þ??`a"â\?Ww">8þ63FGL J0710.5+4732@e8·€4mÆ@6¹Z`ž¦IÀ9mM!À;ÅÉTrH?àÊö8ßx)@ùcãÔP@.0¿æ_p¿åÙLJœ¸¿èR¶ú0:ä¿èhn±í'¿íaœÊrøAGNbllS4 0707+47?ïøc	iØ0?M¶%.8¨?NsÚXŸB?M¶%.8µ?ïQÁ*+6Ó?›‹mKîâG?•ÇÚº™%Ã?›‹mKîâG?ï[¡>'Ò‰?'NµI?"‹Ø-Å®ô?'NµI?íú¼2½¾?ž­ D_q?°*jH?ž­ D_p3FGL J0712.2-6436@q7µ ÝDÀ6*Ð`Ö­À: ²÷8±!À;ÀÀ//˜t¿ûpœ 4=t@£×‹Ê@î¤ûÍ¿Þ{&ëø¿áŠ¡EZ¿æÀ'30ë¿ïÿ§9.8¼AGNbcuMRC 0712-643?íÍ!#ö¿ë?¶C³y/ݪ?±–öàJ–?¶C³y/Ý©?ï»K—1	?š¹Àי…4?-3¹=½?š¹Àי…4?éÿHwi®®?²iOyƒµ?ÈÞ"YEG?²iOyƒµ?ïø¶ŸxnV?RY"Z4?M%'F¦X?RY"Z4}3FGL J0712.6+5033@dÖN wm@7Ûß 'áÀ8èpwa`mÀ;‰þÚf"¿Á<¹Ä²L@F›'{@ºÿÅÈw¿à¯âFdF¿ãE4oØ!¿ßÐñ­Šoä¿âa°¤ÊAGNbllGB6 J0712+5033?ïÿ-¦ªÐV?©RP¶3ö?K*¥õSý?©RP¶3½?ïÑðöÈ]Ò?}ْIT?w"›ÑS?}ْIR?ï­±Ÿ–¼l?…D)~þ©þ?""˜Päí?…D)~þ©ÿ?ïååj™çÒ?aОÿ6Ù0?j•f-ö?aОÿ6Ù63FGL J0713.9+1933@hµ«`kz¢@+/¨þ'j÷À8EìòÝÎÀ;=xmži?÷/Oxä@]‰2C@é¨Ì'jP¿Ü	E"¿å]Xë? ¿åð9cy¿èÓ~XHAGNfsrqMG2 J071354+1934@?ïðwÞ-€È?ZZdg^4K?_C¤þo–?ZZdg^4P?ïÞÖýwùø?y'$Jæ6'?p"D¬?y'$Jæ6'?íèÚ0Ù3?¡l¦Õìå¢?°¿Á.y6b?¡l¦Õìå¡?ïú©;òr"?AI¹¨s'G?E[67xÃ?AI¹¨s'^3FGL J0718.7-4319@oݝ`˜À+Iä ()À8L· "À:ó>FŒ¬K?óL"=@
 wŒSŠí?ýÜ<ŒAí¿Ñ]n€;N¶¿ØÀ¸æÕ¦T¿Øo'§9À¿Þ7F¢?ŸAAGNbllPMN J0718-4319?Þ/\økn6?Êû[KÒ\?àèQƒÊHå?Êû[KÒ\?Բʨ@?ӑÀj¶LV?妚«÷ßó?ӑÀj¶LV?èmJ¿xõÞ?±•L¥czÚ?ÎJÕ(†?±•L¥czÙ?ÉžùÆÈ?¯Å"s,ɋ?é»AœO?¯Å"s,ɋ3FGL J0719.3+3307@g!A?ÐÐh@3Ú¡–'õÀ7•æLГÀ:õ-Iå&`?ù÷ë|eV@i1kÝɟ?ÿº*áU¿Þ=eÊå
¿âdàé©Q¿ãŸ.×·j¿åqî—YAGNfsrqB2 0716+33?ïöyHC~?S1ˆ³Êå?S×
oyÀ?S1ˆ³Êê?ïÛèQ:;}?{åN&¥?r×bâAí?{åN&£?î_ÑýÕD³?žªšƒq7Ä?ªà"«´Ø?žªšƒq7Å?ïõ`6Èì?Xn9ðóö|?Uñ?'n(÷?Xn9ðóöz3FGL J0720.0-4010@oƒT`ªdÃÀ(/&Ɖ½À9à¾H¥‹?À;~áxU|3¿Ñ—=7²¸"@l@ÓVq_i¿è^
¾Å¿æáÐæÊû¿ÑžÀ€ÊQ¿ëUS€I€@AGNbcu1RXS J071939.2-401153?ïÊb«¬$?€Ží"¡P?zÎ÷*)î£?€Ží"¡O?î¤ÈN2ë?¯Ø iuM˜?¥³{ÑW?¯Ø iuM˜?î?hkj? $OtûV¿?®œ	yI_'? $OtûV½?ïYWÔT'%?'Þ4HæB?"Õu{q?'Þ4HæB3FGL J0721.4+0404@j–À_k b@!¼@µpÀ97-m "ËÀ;tù»B`Î?à—Ô¹¼`@þeÿ¹3=@:Þ ‰ÍÊ¿ä
ˆ&ªŽ´¿çˆ¬1 ßI¿è_=Ÿ¸4¿ä-²B£AGNfsrqPMN J0721+0406?ïý½¾2ø&?4Ƈ¶N'?2h>Ô§?4Ƈ¶Nº?ïµ¼†üml?")ým*!?'Þ@ä¥;?")ým*!?ïžhsô
t?"Ÿ<[aÒù?ˆeãü¢ô?"Ÿ<[aÒò?ïµ'ßlG?st%áµbœ?'¶$î9·?st%áµb›3FGL J0721.9+7120@aÿXÿu–…@<ú€d>nÀ6F#ÿ¹‰#À:XG·N¶F?öˆö#2_#@¥É}·ç?ÿ]g1<û¿ÝX¹ÄK7ѿኸÙáïZ¿à»~úÃr¿ã§LºAGNBLLS5 0716+71?ï÷Óõ-)?Yux]cM?QÈX¥¯Ö?Yux]cM?ïÔòÔ?"o\&?uóüþ†•w?"o\(?î°:ù?œ=Iu.'?¤þ¬^þq?œ=Iu.(?ïÿ¿k+ùN?
ÿf?ü,«?%5¬'¦?
ÿf?ü-à3FGL J0723.2-0728@kæù€õ]æ@Á¶@™MCÀ:Z`·Ð¼FÀ;‹Õ`EK¿ìKÈÀE!j@
	†Nc:b?üÅnA&:ý¿ïX9$câ~?ÃEϯ¢'Ý?´ÿ‹ïj¿Ðï‰ôÆïAGNbcu1RXS J072259.5-073131?ïý?ç4:ø?3RCR€‡?6Æ^(8ä?3RCR€«?ï¿tÙÓ4?¡°Pê'?€"ɺ‹2‹?¡°Pê'?ï›AáN?ƒáæ–d?‰/‡œ¬zq?ƒáæ–d"?ïþ£Þù¯
?(ÕK÷=?%Âe5Á?(ÕKö‹3FGL J0723.7+2050@h­O d#–@03ËÿGs\À:Ղ}ô"À;³ÌQ|ÊV?¶ê#A@ËÞ/ ¬ˆ@3i~J‰¿å8'ŽT¹¿ì2ôG"¿ÆàÊv—r3¿ã䂳E‰™AGNbcuGB6 J0723+2051?ïþ•ù(d™?-‡Ê¼, ë?& my¶_?-‡Ê¼, Ó?ïÃÏl±äŽ?ˆ7
‹Pí?~I§
¹·?ˆ7
‹Pë?ï»&×î?€@ºõxq¹?6~
ð?€@ºõxq·?ïÏÚÑÐ?r[ï=?x}'—ðœ?r[ï=3FGL J0724.1+2857@g² ìt2@3[½ ‡_À9¤LˆnÎëÀ;ÄŸþ7©¿îíPzì°@kDDž:@Ác `Ș¿çíí¸nŠ¼¿æu"—™[©¿äßOᔯû¿ïÿï-mnAGNfsrqGB6 J0723+2859?ïÿͳåy>ùîÇ=È·>ù&
Cv3ƒ>ùîÇ=Í&?ïܕëÃ?{Tï‰Ø‹X?qµ}x
ô?{Tï‰Ø‹X?ï¾|/¥?€·gu×?€`ô=Ö¹{?€·gu×?ïýôr|ø?0üº"*'"?0\k"=ü?0üº"*'´3FGL J0725.2+1425@itXf€@+Õà0VàÀ7Z)¤>8JÀ:æWS£ì?ø|§ÎÕ@9ðh2n@ø45f¿'¿á,H›Ó¿ãàNŒ€–¿äXɒ°œ@¿åµØ[4AGNFSRQ4C +14.23?ï鄚€òÌ?hulnŒ‡Z?f{e
49?hulnŒ‡Z?ïãZömu?y[¬µz?lñ¥	'‹%?y[¬µ|?«‰~n?™)Zpl6Û?¥åµGh=?™)Zpl6Ù?ïÿ鉇|>ñ"²sîßî>ævñx"w >ñ"²sîà63FGL J0725.8-0054@k69Àëíú@òÆÖ¤èÀ9EG1í¹À;kÛ._"?»ÍÌçyÌJ@%–¸Öq@'-ÈÈ0¿ä(›	—j¿äŠÔ˯ýo¿Ù+²ÔÍ]¿âr»7½ËAAGNbcuPKS 0723-008?ïì´C2C?fÀ³åÿîÇ?cK¼Í¼í?fÀ³åÿîÇ?ï2œ+m?¦þn¤Ó?™¬ú'a?¦þn¤Ó?ïBlÆêøÉ?'
<•Š?—²g" ç?'
<•Š?îÍêÉ°?"ºþð<"¦?£/A^ƒdó?"ºþð<"¦3FGL J0726.6-4727@p6B 6mÀ,;ý!(n´À8Æ¡ëw²¿À;TwÓv4:?ðMó=yÞ@"rYä¢×@¶- t"§¿â¿:pœÔ¿æÃÅð˜7¿çù=TZ†¿îK7ÛRelAGNfsrqPMN J0726-4728?ﴁiáÓ?}…ž´_xW?'ߥ‡¹Ë?}…ž´_xW?éÿžP¶Ìo?È»`¸±ÿ?Ȇ½$ÎI?È»`¸±ÿ?î…iV? >5{Þ?®Ž®j›? >5{Þ?åí»ª¶.?°ª|SkD?Ô$ˆª"Û¤?°ª|SkC3FGL J0728.0+4828@e2;o@9ÍÕߛªÀ:‹"äþòºÀ;çú#G-¿ú›yhKÃÎ@ÒÍ`Æ@÷ýÀ4¸ï¿êÞÜKðÄN¿à§ê{ož¿ÝDTî™Ñ¿ê<ߕ:AGNbcuGB6 J0727+4827?ïfy7L?˜·òÕ½n3?"-ðÜy†?˜·òÕ½n3?ïÖ&€¢›ª?s‰3qƒ½?tì¿®²+0?s‰3qƒ¹?ìÉÎu|sÅ?­:Iàðãý?¹±ŒTaÊ?­:Iàðãû?ïýZÕÞhé?8MfnîÏw?5)Q¸¹?8MfnîÏo3FGL J0729.5-3127@n¢å>‰©Àŵ ÝDÀ9´I窞¥À;Q¸Æ…Šï¿ë=iöqi'@–'%†ø,@;µ¿j
»¿ãô§¾6-¿êˆØ‰C‹¿í
ÎÖü¿~ǁfûjMAGNbcuNVSS J072922-313128?ïøÛZ%M#?Vñ"é"?L'—jËr?Vñ"é"?ïg2´të\?£֋K'ö?"©qb"‹?£֋K'ö?ïôlÁK?'–ÇæàôR?ž!|gÖ¬?'–ÇæàôV?ïýrÃLÿ?5/#en{·?4iç
˜Z?5/#en{Î3FGL J0729.7-1448@lÍòà\̊?øb½ßôò±À9¾hêÀ;[Sã¬ã?ÖeäJþè@ÜÕô=Ôø@\›`C™¿à±ùĞøK¿èÄxãáo¿ç¿ûö¹Ž¿×L¤•ÃPSRPSRPSR J0729-1448?ïwè0ÞþÆ?•¬Eýh9?'ùä 'i?•¬Eýh9?éÆOùM‰?Ð^V*Sڌ?ÈçšÀÉÛ?Ð^V*Sڌ?í>5Ai'Ý?§¥æ"ßX?¶Uô³q?§¥æ"ßX?ëu°1'•¬?²$¹?Â)?;a©U?²$¹€3FGL J0730.2-1141@lxl_9K{@	Ø_ÒùbÀ6b²<'ÎÀ:l)±ª1—?ø'{j×@m^ÒsTá@¸Æ§Þ¿áapD­üJ¿äǜԷ|Ù¿äç|×I±¿æ£#$a"AGNfsrqPKS 0727-11?ïÑAÚÝY?x,ÐQ)¤Á?w~_'T<?x,ÐQ)¤¾?ï†b¬µ4z?«è÷÷,«þ?ŽgTÒ²áô?«è÷÷,«ý?ízìh?¤oóvïxÁ?´(œ¿äÖ?¤oóvïxÂ?ïý-ç Ð?=±Î	Bë?6—øÆùˆg?=±Î	Bí3FGL J0730.3+6720@b'ºKâ@<™åàš	+À:Xg`ai§À;þÓôß:Ž¿â<žüÚ܅@¤­'ÊÈf@ëø :G¥¿éÆB+ôz'¿äòíVkWοèˆ(»`å¿ïÿl³Ì9™AGNfsrqGB6 J0731+6718?ïíäؤ?aí›9¾?b'[ãÿ¦?aí›9¾Ž?×ìá?¤ ß1îi?Ÿîk…cÓ?¤ ß1îj?î¡ñö0JY?˜ª8t®§A?¥ààœûZl?˜ª8t®§C?ïT
ÓÃ#û?ԅ[‹(?•~E‡›€«?ԅ[‹(3FGL J0730.5+3307@g;öÿ:Þ"@6e>‰©À9ù>
ÈÂÀ;̐"£¶¿îvº8—îk@2ˆá:˜@ïý |¢=?ÍØ¢òŽ0¿è䴲Ϡ'¿ßÆNdMBº¿ÓŒÓ
‡ #AGNbll1RXS J073026.0+330727?ïú~[ÿk?Hd†G¥Þ?FÊO{?Hd†G¥Þ?ïØQíEÜ?€°ãsoî?s×	]ñ]?€°ãsoî?ïsß,Ýæ|?‰SçÙÌZ?'"dC0—?‰SçÙÌZ?ïøÜÓÀi?NÊôÙ¨â?LŒ°þ[³¸?NÊôÙ¨â3FGL J0730.5-0537@kÍóFí$@C·À AÀ9ÃÁð8À;Šf¿àîð…†	@Ä:ø‰@Í쟥ø"¿æSñÜѧ¨¿ä´Ä16ž¿ÅÇ$%hA¿êèˆ±ò´AGNbcuTXS 0728-054?îë/ZV+"?¤naFç;?¡M
ZMÚ?¤naFç;?師1?¡D{2uï'?ÕF'Õ4?¡D{2uï'?ìÕ¡ð¼ã?§»ù:ƒ4?¹W'ðzë?§»ù:ƒ3?ïÕmøÍÖ?uŒ8ãE
Þ?uIô™û?uŒ8ãE
Þ3FGL J0730.5-6606@qZhŸÆÚEÀ4Õ  0øÀ9ÑwÛðuÀ;‡±ñ\Ï¿ï;¹ñöw@
»7
³Fê?ü 4á368¿éÇO á¿Ø´–×ꯃ¿Á! ]FñÆ¿Ý8úÉpˆAGNbcuPMN J0730-6602?ï÷›DØÓ?SîÚùXaR?PüÉvNY|?SîÚùXaR?ïÚýS'`?€4²9³?r÷V>Ïé?€4²9±?ï·Z¥à¼?{Áߟ{Q?')V‡úQG?{Áߟ{R?ïý@K‰\v?:Dâ~h.Ñ?5ý£µY˜?:Dâ~h.ª3FGL J0732.2-4638@p0Ã?…Q
À)ÌG¢'vÀ9e¾/áoÀ;làæ_E
?úÜÐ*zR@šWÍ|2@)ë‰%ƒ¿Ø8qÂKOÆ¿æ¶É ûì(¿îýØP
´t¿ïýïmqٝAGNbcuPKS 0731-465?ïàÉmD?˜s$ÎXå?ˆ¹Gͤ¯5?˜s$ÎXå?ß@wœ•2,?Õd/M;ôõ?à_Ä1µfê?Õd/M;ôõ?èÇ°±eÔ?²»+z'{n?Ìá?µ:h²?²»+z'{n?Ðm¶bêÚ?¹ÁQ¿î¤®?çÿI$Ί"?¹ÁQ¿î¤®3FGL J0733.5+5153@dÀm ‹]@;Vš ¨4À:pÚ7›À;×5Ú­` ¿ÏÐqûxf@
dÈÚ#øX?ûÚß?ãýb"Rf?èòKÅXí¶¿ã¬[ñ"׿½7'lÃf‹AGNbcuNVSS J073326+515355?ïR+#¨õ? ÏBŠÛR?•º›Šða? ÏBŠÛR?ïµwè+«?ŸÞlםæ?'¢õ9Tû?ŸÞlםè?î¢ö 
Ž?›S ¯_?¥ÐÿWE?›S ¯_?ï·yƒ¦R?ƒÂ~D
§æ?'!ŸëÍ?ƒÂ~D
§è3FGL J0733.8+5021@döè ÓI¿@;½°ŸpÀ9Å»{k±)À;Òîî_Č¿ñ§fiœ@îKAFò-@¾ÿ¯£¿çúÚâµû¿æª¢_)Êî¿çCÑ`&Ó¡¿ã-ËÏAGNfsrqTXS 0730+504?ïÿwѨÉ<?8ÌJYN?Êæؒ‡?8ÌJYh?ï×ôÑ/?<?~vrÝTÃâ?t—h`b?~vrÝTÃã?ïÝH䄣†?ojҁOùñ?q[½®<›?ojҁOùô?ïÿz.k›y?K¿€â¡»?º2Œ¹V?K¿€â¡¿3FGL J0733.8+4108@f7)à¤&@9
ohیÀ:.ήN\"À;ê‹y¢ƒ? ¨8t¹Ûñ@
(2F#Oæ@ÆÎ`u¶¿ì˜î
V'€¿Íɉ¬¿–¿áf`­G~ø¿×¶óËØõ¿AGNbllGB6 J0733+4111?ïäYýš?p`S/ìÏ/?ké¦ødÙ?p`S/ìÏ/?qp4?'{!'¬äÔ?ŠÝc¼#òë?'{!'¬äÒ?ï,"V·™-?"âÐm­?š{µ)ÚO?"âÐm­?îúÔEž?"έÊ%? R»§/F!?"έÊ$3FGL J0734.3-7709@rŽ¿ìºÀ8(àÉÙÓÀ8аô)2À;n`TÔn?é"tþžoÜ@H50cu@R'ıJ¿Õâ°)åù¿æHû*‹¿åðûDU¿çq$Ê(œpAGNbcuPKS 0736-770?ïûUÅoPò?Aš ú"|?B¨êB¼5?Aš ú""?ïÃxÈ®Ú?‡¸Îåï:
?~C›¨ñ'Å?‡¸Îåï:
?îv›:+Z?›ñîë¾ìv?¨–LWíJ]?›ñîë¾ìt?ïV®ñB?…7i3e?•>*?¡×É?…7i3b3FGL J0734.7-1558@mž@ÈG,@ž 'ðÙÀ7⥤i×4À:÷ì^òÕ@™ãC0×8@²ß¢<€d@"fx/º¿ÖÒXbËt¿ãAVÊŔ'¿è%n+¬¬¿íì¹®€PSRPSRLAT PSR J0734-1559?$W=›ïÈ?!Wኡ}â?ïþºŒ&Oò?!Wኡ}ã?4
8åé²î?MúÉ0÷ìˆ?ïý~XãBÊ?MúÉ0÷ìˆ?…Nÿv¿p;?}¤Ü?ïªÄ%??}¤Ï?.¦6¤·Z??(4ƒg³?ïþœ•´‹?(4ƒgµ3FGL J0738.1+1741@i;dÀßXÁ@2'ŸªTÓÀ7"^™éJ²À:ÅD1ˆ8H?äëWÒNí@yéØ÷'"@
?·¥ô¿Ü3†Ç¿áÏ-à8¿Þñë²7—"¿Ü»ã"$VAGNbllPKS 0735+17?ïþ9ÁC±?'Rfš]?,cëÄî8"?'Rf™É?ḯ²TH¾?'0°¦Ð?y¿&ÕÛ¡??'0°¦Ð?ﱚ¹³¾è?†˜*MØgå?ƒ™Q"F2?†˜*MØgì?ï§ÛëR6 ?€¢Kœ‡+?†	+rX
?€¢Kœ‡.3FGL J0739.4+0137@kËßÒc@&е~ÒmöÀ8%W¨]'À;T»ÉoJ;?û$G%Ž@>«6z@ SMÚÔL¿á𗳡"Ê¿è\·€à:=¿çËíSÕë¿ìÆ©C'ŒAGNfsrqPKS 0736+01?茶z
°?'0Q-ÚîB?†a|}TA?'0Q-ÚîD?ú;¢Ç?³¼Ô7Pçï?¦6à\EÓv?³¼Ô7Pçî?ìغßH<ø?§7ï•êsÐ?¹:)¾??§7ï•êsÐ?ëg‡7$ÊÙ?³oB8>‰·?Âaã#lԚ?³oB8>‰·3FGL J0740.8+6621@b¶°À&Ì@=œzߚ.ëÀ:frû À<Àu¦uJ?õ»½ ´ëÛ@7[íçy¡@1Ø@žUÁ¿æ]¢ÿ/0Ö¿Ñ~"´Ç6O¿æ½"e¹ú¿ïÿïÝÚ!…PSRPSRPSR J0742+6620?ÒLÿæó$…?Í!ÛE€£?æـ†m½?Í!ÛE€¢?Ä|ÿLU?‹­:ßÄ?êúàÿ@,ë?‹­:ßÄ?ÓJº@$B?¹&‡d°ˆ×?æZ¢ßíÞ÷?¹&‡d°ˆ×?ÅPrwiA?±*ÕN•=?ê«ãb%¯¾?±*ÕN•=3FGL J0742.4-8133c@r]…À3aVÀ8ù_{šÀ:ÃÃX¯Ä~À;»‰'ä™r¿°º"ËZ…@	Ü=IaÕ?÷l?¸ý¿ì‡/ÆäwܿٓtvŸn›¿àÁM<ɵ?Ø2E-¹AGNbcuSUMSS J074220-813139 ?ïý>XJ/Ì?6w½øòM…?6
=®šZ?6w½øòM?ïá_¿¸ˆ*?wÕ+ºMô?n @GwÔó?wÕ+ºMô?ïo@ß¿›?Óa¢/°?'×ä‹?Óa¢/³?ïà"?nt×~††‡?obkðýß;?nt×~††‹3FGL J0742.6+5444@dam¿‹›ª@=Œ`Ëò²À7ÅÐÂû'³À;3ÁÑÇ'?÷¿n2†@È8'ŸT@(ªªŽ—¿áV£Ðª'¿ãôIL
€É¿äŸ&ãæç"¿èU)ßÕòAGNfsrqGB6 J0742+5444?ïñÃQ%?\Á­,QT3?\y]É´á½?\Á­,QT2?ïÛQê¶?z½)ï»U¼?rW
Àp%?z½)ï»Uº?îUùÄ÷ÚT? 9[3Õy?ª c°'ZÅ? 9[3Õy
?ïÿèš'>î}Dt4ð‰>ç€eão'¯>î}Dt4ï3FGL J0742.6-5623@pÍN wmÀ/c1àLÜRÀ9Ëú/ÜfžÀ;£'ð	è·?ãmÛç-1x@7º¢Rв@n[à¦sr¿èV€G솿âM.6c¿ïþœ ::¿îŒxϨ'AGNfsrqPMN J0743-5619?æ±½[*­?ËsJX†CÄ?ҝʅIª¦?ËsJX†CÄ?æÎz™H›?Ñö#š2I?Òc
ÍñnÉ?Ñö#š2I?é°íp­lŒ?±IG7Ž£!?É<J=JMÒ?±IG7Ž£!?â&å1"7?ºŠ¯}Âj_?Û³Ô5œÙ'?ºŠ¯}Âj_3FGL J0742.7-2824@ny)Ÿ¡—ÀÎE s'•À8àa'ÑÖøÀ;!º+àX›?ö¯þr·,§@C1.ãÃ@íèô>׿Ò&'Z¶°¿äíî/ýW¿êàŧ‹í¿ïL3íÙPSRPSRPSR J0742-2822?¸‡e?ž»£Ûö]~?ï?w3Ç4?ž»£Ûö]}?ïܯLö)?©ú`!5N?ïˆ@BÌ)?©ú`!5N?¼%À)GWÁ?«üË^"ƒ ?ì{Gú×?«üË^"ƒ?³at…f‹?˜Í žM+È?í"Ño]3.?˜Í žM+É3FGL J0744.1-3804@oŒ-@ªêûÀçÆ«±ÊÀ9®œ­JP†À;@R,†q¿£Ì0ú&@
m‡Aþ'@q³?ˆ?¿ç¼d™Ì¿æÐ9Ó$C›¿ë3@ð=ÈÁ¿ïÿ+‰/OAGNbcuPMN J0743-3804?ïZÖú¦??™LÂFNŠæ?"¿ «83?™LÂFNŠå?âëýs?Ô<6Æî3¯?Ûô)ñÒ?Ô<6Æî3°?ì©æ
ٖ?¦3ã¿ì"{?º°Ï—ù3M?¦3ã¿ì"z?臠ºŒõ7?¸Åb9Ÿ?Íá}Ì+ ?¸Åb9Ÿ3FGL J0744.3+7434@aˆÏÃø@=–²ß»¼ÚÀ9Êìˆ3@À;Ô=ß^ŸÉ?ًž`Ë\@Ú6n&#U?ÿÉ¾Ð_Ô¿æ
ÂmDÉU¿è¿²sð‡¿Ñ]i4'пƧrŒ¤AGNbllMS 0737.9+7441?ïÿ+žI¿«? ²¾(gw?Œ6È
¯b? ²¾(gã?ï͋6AÒ?'G†Ž¿·ö?y:väß#?'G†Ž¿·÷?ïéxNnæ–?oxì	"²=?f‡±'iÒ?oxì	"²B?ï偛ΤÖ?a1t]ÀH@?j~d1[*a?a1t]ÀHC3FGL J0744.8-4028@oÑÞß)À 	ÙÀ%I'À9cý!(n´À;RZ8Zº?åä68@
h/žÿ	5@·[à{€T¿èø-®d¿Õ^Ž1퟿äC†Änž2¿ïÿž'ƒ© AGNbcuPMN J0744-4032?őRí»s?Ç(
ü
×}?ꛫD'#;?Ç(
ü
×}?°s"Ö •?»CÆn*ÂÝ?íñe+ýM?»CÆn*ÂÜ?֚ë¸ÕNX?º` £Á)D?䲊#•XÔ?º` £Á)B?Ìشlj?´±ëTF‰û?èÉÒξº?´±ëTF‰ü3FGL J0746.4+2540@hWFà!q@6Ø1ôoÀ9MC%¾=À;¨¤Ô`?¿ô¨cpŒ@üç¨eÝ@¶šà@œþ¿èÎíd?οêß"Œ"Dè¿çO¢D
 ¿ïÿû
LàAGNfsrqB2 0743+25?ïÿ¥xUá?C;ïŸ?¡ê¹˜æ?C;îÕ?ïÕÔaÅ :?€òÒðØÎ?uÏoã-?€òÒðØÎ?ï[o(Y¢?Œ,ᑥ«?©$5é—t?Œ,ᑥ¥?ïüÚpièà?@Lãfw"?9,|°¸÷(?@Lãfw3FGL J0746.6-0706@l6Èó#@!½•`$À9þ!ã–¹À;kfKŽt?Õ:[¬ñ@ºÁeæcÍ@‡Â yÒ?ïìkü'ƒR¿å›Üc‡}§¿â÷ˆ"¢Ø¿êøÈ¥î(AGNbcuPMN J0746-0709?ïìYzDå?p7Ê<2wÊ?c¦…»ðY?p7Ê<2wÊ?ïD›/t?¥[S‰O±?—lÚ'¤?¥[S‰O±?ëö@Gù!?¬ºÚ€adõ?À'ªþàz?¬ºÚ€adô?î†ÙéÏS|?–›N[ܙ?§'ac
È@?–›N[ܚ3FGL J0746.6-4756@pUÕ`"¥À&¢ù;.ªÀ8øžâ®¶aÀ;Wƒï
iu?æüEH3 k@x¡Ú±@¾_쥿ç®(&ÃA¿äãˬfOë¿á%]èÇî¿ÖM¹º1¦AGNbcuPMN J0746-4755?ïòÝùY8?`ßG2¶Ø?ZD
áM`?`ßG2¶Ò?ïe–R³åx?Ÿ$EQkÓì?"M5©ƒPá?Ÿ$EQkÓí?ï/X
¯Ñ?'…ªk{I_?šþJ?'…ªk{I^?;Í?"í§'5J?¤OOìC?"í§'5J3FGL J0746.9+8511@`à·ö@<. Eð¥À:/(âwYÀ;ÐÍ×°VÀaK:»è¤@ïàÚñ?ü˜ì€Fac¿é™'Xßj3¿à&ÀøÇì¿Ö8ðÐÞg¿ÍÅaðA¶AGNbcuNVSS J074715+851208?ïõ]Tü™7?\
>ô?UEV͒e?\
>ô?ïÜ ­âè¨?|nIã»w?qï©‹«ë?|nIã»y?t¾$?…³aú&ˆ?ŠœbÐvüB?…³aú&Š?ïÿމ8àX?Åã·ZÙ>ð»cÔ*Ñ?Åã·[a3FGL J0747.2-3311@o
•$ÝÀٟîó=À8ƒjƒ+™À:Ø G2Ä?Î,Ùx'ôö@S­|$"@y¹h¿â50hJ
¸¿æNíìW+¶¿å)‡ZID¿ä…R\Ä&5AGNbcuPKS 0745-330?ïè‹ï‰H?n—p[Q<š?gtv¸Ø?n—p[Q<—?ïClÇî+Ä?ª¶´ƒŠµ?—'g:‡?ª¶´ƒŠµ?î—9ù{?ž֍½´?¦ŽÌ`oˆn?ž֍½³?ïõ©Ò©Ù?N}dæj?Uø¬Z¬Oœ?N}dæV3FGL J0747.4+0904@jb`RP/@0ˆçÖyõÀ:d%‹ªÃŽÀ;àК·§?âˆéߓ_)@Hî=à¶9@‡Â?ÖØ¿ÛB¦¿X+K¿Ó $ØÒiš¿àø°ªF(ó¿ãðsÚ AGNbllRX J0747.3+0905?î˜Y¤ë
"?®]ª%ø2›?¦ze±O&²?®]ª%ø2›?í«øÕD2L?·d»Qº?² 9UÞmž?·d»Qº?î&žàJ? ¥'‡†?­–þûV5? ¥'‡†?åÞé¦ü/ä?ºå^Ĉ@?ÔB,² ;?ºå^ĈA3FGL J0748.0-1639@mF÷_²íþ@ÎÙãÀ9/Ã¹þ"À;CÖS^Kæ?õ–qÆì¹@ۖÛúT@Ö[ 9ÆË¿â
^¿èGCˆb\¿ì˸0F¨¿æ@ºr'(AGNbcuTXS 0745-165?í*ÙÛ9`~?´UЦ¹X?¶©1&4ü?´UЦ¹X?è)Ià°?ÓÝóšD?ÏZØ}˵>?ÓÝóšD	?ê&ò//T?±iä³Pî3?Çd7CAú´?±iä³Pî3?ÖK§WºÝ?½æ¡áˆœš?äÚ,uT"'?½æ¡áˆœ™3FGL J0748.3+2401@h'FŸ¸@6­?i¢[À9ÀÜ0À;³Ô&]aÛ¿ð ~ðËډ@[µàÏ8@@`k&¿àñðj¿ä,fꉏû¿áéñd '¿ÕÙ°"AGNfsrqS3 0745+24?ïÿÒJ@œü>óI‰IëO_>öÚß±Æ{>óI‰IëT·?ïà–Œ€î?xàSŒÌxø?ois~ä?xàSŒÌxö?ïތè^ü?wP8Wî¤?p¹‹¸P'"?wP8Wî§?ïÿéá•e>æ.ÎóEÚ,>æjùšÇ`>æ.ÎóEÜj3FGL J0748.5+7910@`ß2_c<æ@=GÐ@ÔÀ:›OC427À<)LqMJ?ñj®òÇ2Y@£àÒ¾(o@¿ï©H8?Ñõ%†wRó¿ãæZû#L`¿ç«Gþ‹$¦¿ïÿ¼rÙÞ¦AGNbcuJVAS J0750+7909?ê¼*¬ß?ÍP¿› 4?ÇýW'L‰?ÍP¿› 4?æªÁ šK¬?ɯJ¶öHê?Òª}¾Ëh«?ɯJ¶öHê?áVßiœÂ?»˜J;̵?ÝRA,Æ{à?»˜J;̵?ÜMíÒµÂL?r#ő?áÙ	¥Ú?r#ő3FGL J0748.8+4929@e$¯ÿ6¬d@=XlÿݛQÀ:3½äÒ}À;âÅû!?ևæ³þŸ®@
­ÍŸZ£»@¶jyÍv¿ÞíG€ù¿ã©;ˆAWŽ¿å¦ÐWN¿îÑzÎþ*hAGNbcuNVSS J074837+493040?ã!]àIìï?ʉ×Ô¹ë!?Ù½D?l&#?ʉ×Ô¹ë!?ènxÌmb?ĊÔªd?ÎFÏâJw?ĊÔªd?éIuü©.?³cÊñJ¹?ÊÚ('[H?³cÊñJº?æGˆúÕ)Ó?·täÎ[?Ópî
U¬Z?·täÎ[3FGL J0749.4+1059@j/
€CR@1˘<eâÀ:¬ÿiÀ;¿­Aí
?Ôpw%?C@™#îq¸)@ŸÈ_ÂX¿ç&J;¯Ðà¿Ý•tè—A¿ãVòì'Zõ¿áKâù×>AGNbcuTXS 0746+110?ïùwØ¡*?S@,4žG…?Kþ {\…?S@,4žG‡?ïʀ7ø½?Ezñ­Ø?z¿äñ!¾?Ezñ­Ø?ï¥ÿ±â?"T¦Ð%±q?†€ºþµ?"T¦Ð%±n?ïi*ì?ƒûTgĖ?'Ü<þú¢™?ƒûTgĖ3FGL J0750.6+1232@jì O*à@2»`c'À9c+Hƒ'À;pClfZ¨?ë
ªj³c@VF,	HS@J:Ÿäƒ¿ÛTÌÍ+J¿éX¿Ž˜+'¿âßã鰝¿è Ü/&šZAGNfsrqOI 280?ïþØJEb?!¡Qk r?"{_©¿Î?!¡Qk r(?ï΅'œÿÂ?t`rÁM(?x½>±€ 
?t`rÁM*?îûŽªšš?–-è×û±? G%VV2?–-è×û±?ïe½\Ë?("Éåg?"H\"fµ?("Éåg3FGL J0751.2+1806@iX;o@5ÏÀ¢À9Ò»úÀ;¨•Š@`B@†äÇ@ïßq<X?ûxt=i—ô¿Ú"DPo¿ÓˏNÖÁ‡¿ã^;÷š¿ï!Õ2!oPSRPSRPSR J0751+1807?`ÞþÎ&Ur?W>¯åNÚ?ïï!1Ù«?W>¯åNÚ?{k,'¶é­?ˆÃçü6)?ïÉ)¦Ú'.?ˆÃçü6+?‹Þ'aÿA?c—®)ç?¶x"?c—®)î?rw¨™ë.?n6r*?ïº6!]˜R?n6r*3FGL J0753.1+5353@d†A¿½ð'@>…Á?ÐÐhÀ9?ª¹|ðÀ;¨"?…J¿ºÆ^;Ó|@ ®÷#ã@ØúÀP»¿Ñ•º'L¿ãþ-Äx.T¿á5(²7Œ¿ß_~þ°AGNbll4C +54.15?ïþš+ž´ë?'xÂçQlµ?&]F±[‰?'xÂçQlð?ïÉǼáŒ?'é£~­®"?{!¸9ƒ?'é£~­®"?ï¢Fºö.?ˆYÑö`²¡?‡{.QBt‰?ˆYÑö`²¥?ïܲ?*?eЇ^£¯'?q¦àjø²Q?eЇ^£¯™3FGL J0754.4-1148@lÙ)¿*å@ y–ÿáL6À8¾2lcÖiÀ;CÉv7]?êÅÐsYN@—M·B÷Ì@á©`6 £¿Ø@)vý¿ãsQŒË¼¿ßMJ!G‰"¿âª¦žS¬iAGNbllTXS 0752-116?ííaî?¬dêjÞ%?°—?ìð¸?¬dêjÞ$?è^:i^'9?Î^i	h<e?·Z…»?Î^i	h<f?ì@M8¦Ë…?ª;¡àÚ?½ý–:É£Ø?ª;¡àÜ?ᔘÃ8B?²vÁÅÍy?ÜÖÎy{Õ?²vÁÅÍz3FGL J0754.8+4824@eQ4 -œñ@>(l <K
À9š0˜N@À;ž"Ž½ž?À¬ÔOß!Ÿ@!eÁzß@$=ÿêÜW¿àêø2†K¿âÏØ°ZÑ2¿âTSK×nç¿ã»´0É¡tAGNbllGB1 0751+485?ïëH^سµ?gaÚþœ?d·¡'LKÔ?gaÚþž?ï(—±»ã&?0ʈO*?ší	ȃ›{?0ʈO*?îæyúÔÇU?—·湁g?¡˜`R³Š¬?—·湁i?ÐZÎ{?™Ö4àéÙ?§´'úSG?™Ö4àéÙ3FGL J0756.3-6433@qTR_ét£À1Â\ÀË6ËÀ9ޟð˯–À;³x«ˆ¤¿ÞtÁ' @atÇ},¦@¼T@(4¿ä"ôµ¸Î¿åM7È2"+¿ãW'Ñ_Ú¿Ù+Ҋ뚲AGNbcuSUMSS J075625-643031?ïû'·åDS?Cw
‹õ&@?Aµ jî¶Î?Cw
‹õ&P?ïȐ÷VÑi?‡!ôƃût?{·"T—L3?‡!ôƃût?ïºÖFþø•?~Œ×Š'¥s?Jn@AÚ¡?~Œ×Š'¥h?ï竉¾·á?_ßM[Ÿ]=?hTvAHG?_ßM[Ÿ]B3FGL J0757.0+0956@jiʞõ#-@39 4¾NÀ8"ÕϪ͟À;W4H)?ëÇ:
V´Ü@"Ë'Rz@trŸYÌû¿ãàN#Ïh¿ã£dÃüÆ¿ãq
â秿ã´^zù_AAGNbllPKS 0754+100?ïý¬ø'\ò?3ýäYìÁ‹?2˜>Åh0?3ýäYìÁW?﫼àŒY?Œ–$@ý?…9PÇÜéS?Œ–$@ý?ïwý¬1Í?Œ´BnÄFˆ?'J¹Æs?Œ´BnÄF"?î"DfVü¿?"ÚÜy"æ?§»¹š4?"ÚÜy"æ3FGL J0758.1+1130@j=ÒàãG@3õ[_¢'À:_Y²"ý[À;ÒNér?çMÒ%U@G®¡hšô@QFt›?à‹!Ω=H¿çM>Dð[¿Ò@bÒn]'¿ëJ¥mQ+AGNfsrqTXS 0755+117?ï
TØǏÕ?¥á–{,£?žUdçM?¥á–{,£?íÆ·U;P÷?µÈp¨¾;?±ÊEV%xJ?µÈp¨¾;?ìá}ø?« 'ã{_é?¿ ôL??« 'ã{_è?éÎPbõ?·ú&<t'e?ÈÆ¿"ªt,?·ú&<t'e3FGL J0758.7+3747@fÕø -à@<àu¿Ÿ½ À:—±æ—y.À;û>ß8à¿ÓX¹mR‰@sŽíï@>¥ 5"?ç‡ShTJ¿á'[ËF©¡¿ärÜDäá¿âÅz·pAGNrdgNGC 2484?ïíÙ£Ýfl?l§ÎGçf?b&\"™'Ž?l§ÎGçf?ïÅÛ<è™î?Šùìhµ?}a‹³L?Šùìh¶?îÛ"Zï(?šäŸ
'?¢MÚW!
~?šäŸ
'?ïÙ…m?j%ló
€?ss=~ÉÆ?j%ló
{3FGL J0758.9+2705@hI#ßm¹A@9òσ³~À9ù"'Ñÿ<À;ÓËwb7-?é]:êGî@†lQöÃ@ —пæýGÜb–ù¿Ùæ×Ê°¿Ü7£8Š¿ê驀'¾ÇAGNbllSDSS J075846.99+270515.5?åýµ<íEï?È6¼Qöym?Ô•†%t!?È6¼Qöym?ݬcöXt?ÐRßÁH ?á)÷NÓÇ?ÐRßÁH ?çÂ}iš?µwÙ͸r~?Ð{ÄÅ,Î?µwÙ͸r~?Úo$o\]Û?·—×fãñ?âÈmÈQÑ?·—×fãñ3FGL J0800.9+4401@eø6ŸÏ=À@>‰M߆ã´À9ë̗ó§,À;åáMQ?áÎn"w	¼@
dSÉ&@X?Ý»¿àJÄë	¬Z¿ãžK'gµ¶¿ã•ßû¨­^¿ëǵn6itAGNbllB3 0757+441?íÆUÊ¥Ÿ?°‰>ôÒ?±ÍQ¯ÚÓ?°‰>ôÓ?íñ̒£½'?ª–f¨Ïk?°q›jâm?ª–f¨Ïk?ëñÇÓ-Ù?¬tòóÚã?À8೗H™?¬tòóÚã?êÆ}ÀK"?¬Ðå£Du?Äæÿ¾Ñò?¬Ðå£Du3FGL J0802.0+1005@jw6â—@46'ßk5À:`2g[XìÀ;Ô:0}vM?ÓÈì²44@Œsk\š@*‡?Ïε?äø‡ç2¿×õ)¹Hß¿écí°r#3¿Öåæ<2AGNbllNVSS J080204+100639?íK÷Þ²"$?¶Þ"`tÇÖ?µ A
kfé?¶Þ"`tÇÖ?ïr¬ü? üç¶ío?'¼Ê} |£? üç¶ío?ëÙÛiŽ–á?´I¬â·B?À˜'YŤ?´I¬â·A?íæeû×7?£4¤Â$e?°ÏTÐ!FQ?£4¤Â$e3FGL J0803.3-0339@lƒ@'À‡@,[	 :2+À98'ódKÀ;kՙ$(Ô?ÓNЦ(ѹ@÷êï!¶?ÿðÁ¡J'ö¿à<ÐÀ¼¿á6‹ÐêO¿Úx¯IÑ}¿ã&oI¨¯PAGNbcuTXS 0800-034?ïýKƒ¢…|?4õ::µ>C?5£âëÔ$›?4õ::µ> ?ïÌɉýt?'ÜKÊß?yý;F*?'ÜKÊß?ïÃÍjîÉA?Žï¯c­k?~Jˆ›_Þ?Žï¯c­i?ÀèŒ?z!ÌïS?žÅýÜ÷?z!ÌïT3FGL J0804.0-3629@o¡œýç!À-ŸöUÀ9JⴕžÀ;êßÝJÉ?ôUi"í];@>Q%âg¿?ýAŽàØóL¿ãw»3®i?ïõÝà£÷Ê¿Í@X¤u¯s¿âŠ­)楳AGNbcuNVSS J080405-362919?ìÊ*fqE?·3áîÇzô?¹®¬Ìwõá?·3áîÇzô?ä˜GÕå™?Ó@.uÀÝ?ÖÏpUø4Î?Ó@.uÀÝ?êؗy¸b?¯ø"w"T*?ĝ£¾v?¯ø"w"T+?çOçÑ3û—?Á6Õy Á?Ñ`0]˜Ô?Á6Õy Á3FGL J0804.4+0418@k/òÿÑÜ×@2/ Z8[À:9Íp`»,À;Î ž9%¿²ÿÖÈû¼6@bÎ
{@‡¾?Á6¿ám, 
樿ìSò²ÿ¿âu-yÆH¿ØŽV,\AGNbcuMG1 J080357+0420?ïÿšPÐeÇ?«U†"n?	kË掲®?«U†!Ï?ïÚ=¸°˜?|ÇAãv?rá#§³ð¡?|ÇAãw?ﶮ±ÛÖ?Ñ™a!܋?'TzS‰
;?Ñ™a!܈?ïæƒ
¹?bÁãµ9Íe?iþý|òE[?bÁãµ9Í_3FGL J0805.0-0622@lj	 'RT@*iݾŒ˜)À9Ð%E3æ·À;sŠ÷?g¿¹QQŜ6?@(©€—j?þQìa<°à¿î~»Þ?Š¤›£M¿â½Y4N¼&¿Ÿ+ÍÊ^ï‹AGNbcu1RXS J080458.3-062432?ïüà>ª¸?5ÚÛÁfôA?8þ'ª9?5ÚÛÁfôV?ïÝ!/¢'H?z‹ÄÃÄU?qoh.ì[g?z‹ÄÃÄU?ﶠŠzœš?³_lŽPŽ?'WÝaXÙ3?³_lŽP?ïòæ	1óÜ?ST*•D"?Z3íœGc?ST*•Dƒ3FGL J0805.2-0112@kÖ3?Èlì@/—(_ššKÀ9"ÛVÓKÀ;¸Y_æÌ?àBñ¿þæ®@?ìsS4@·ô`d™³¿Ùv'D"E¿è4îV,¿áÄìÿUK¿è²+¸YgAGNfsrqPKS B0802-010?ïþMª˜4%?1µ–́ló?+%V|½¢œ?1µ–́lÛ?ïÏVl'?'x1:YÖ¤?xpÔôÉí?'x1:YÖ¦?ï/õ[Ł'?'ÑËÓ#r?šT‡OÍØ?'ÑËÓ#o?ï¿æâÛ_ê?r|üó´HQ?€GI(_?r|üó´HQ3FGL J0805.4+7534@a\j~ùÛ#@>ʙ÷LÀ8Û+6¯ÆÀ;s}°/U¿ú'Cß}Ôl@;ôvH?þ®íÿ!ˆ¼¿ÙÁ‹EmóN¿ß©Æónø¿ÞMdâ­µ¿ÑkFÖºG AGNbllRX J0805.4+7534?ïÿ^!­Ëã?WP‹R¯^?;ÊFƒ¦?WP‹R¯u?ïÙt2דã?€LI"¤·?sEæ"6
Œ?€LI"¤¶?ïÏ'eNjì?|Hçœz(?xlM:	+?|Hçœz(?ïÿëiu©>ïÄî#Õ¾O>ä–pŠX2‡>ïÄî#Õ½3FGL J0805.4+6144@caA?ÐÐh@@.é€aº/À9öåvÀ;ãe§ú…m?ôIYÑÇÞ@_!CœŒé@üº€™îS¿ãã•Vœwx¿ëo¼™Ï¿ëÔ5™6j¿ïý2È1æAGNfsrqTXS 0800+618?ïöèî8†?Wü÷ϸÊf?R.#ÎóY?Wü÷ϸÊj?ïÀ#¹[?…ÔÑ{U?ðnu£R?…ÔÑ{U?îq!\0 ?ßc¶‡^´?¨íî
<ö?ßc¶‡^´?€?ƒ$…>?Ž_ý;¾¼?ƒ$…>3FGL J0806.6+5933@c³û_ïJ@@J˜?ýFÀ:c/Çmè;À;ïÅôkwGÀ`
+Òí@(õgJ¼è?þ€W([¿ïòÌÒÅÎñ?ïK™™C³^¿ëĎ*XKÏ?Ôb­WD=$AGNbllSBS 0802+596?ïÔøݾzè?|/Ôìó<Î?uƒ' ŒŠ?|/Ôìó<Í?ïÖ庽£§?"©WCs?t"¡.,^?"©WCt?îˆçôÄô? _±4;¶s?§q€³¾`½? _±4;¶t?ïÿõ"¨ÌO>ñ¹2š"~½>ÔØ®g`>ñ¹2š"€3FGL J0807.1-0541@l_?p]@,Ï¡"cÀ8Ât=¿~0À;BñTk'?ðM¥&À‰@2^?Pwè@‹°ÀQ¿:?ɒ˜Y¿àŠÚ‹É™´¿àÙ"v€›¿æB£•4ÉÐAGNbllPKS 0804-05?ïû':Ö¹?@ßÙiœÖ?Cc¥~?@ßÙiœÍ?ï~ËÂæP?•â$^…:Z?<&‡£6?•â$^…:Z?îÁ¶ÃD{Í?šíǓï?£ä"˸C1?šíǓô?í=*LFs?›ïíÓ.PH?¶«…Ìs?›ïíÓ.PH3FGL J0807.1+7744@a
¿p@>tþÀdß~À:*‡{‰äÀ<D™`¿é×s¾àóB@Ë,çêŠx@}/`jÎÖ¿è°—YoÕ¿åô©Ä\ß¿æµ´"xít¿â
¢ûd‡6AGNbcuNVSS J080637+774607?ïþÄ 
O™?.›ÏÓáŸ?#µÿ['?.›ÏÓâ
?ïÙÏô"J?{‰ŒÁJý?sÀnۃ?{‰ŒÁJû?àQZ?ŒŠ#µA?ˆÕ똩Š?ŒŠ#µA?ïý#ç¹?5ð™úÈÅ?6ãÂ7Ê´?5ð™úÉ3FGL J0807.9+4946@e'ŒŸ¶M@@9»üÊÀ:$B_öàÀ;ò©1½n?ámyÜK@Q'H—sz@"@ªÀ3¿âœQ:7çÖ¿ãlº4ç	Ü¿ïÿô³à[¿Øùå!ŠòÀAGNfsrqOJ 508?ïðc©¨}?zôÎ0xæÒ?_8¬¯é|?zôÎ0xæÒ?ï2¦Qƒê?¦+œÄJ"!?™«5ς¾?¦+œÄJ"!?î¿Âg­q?œ1Þd¤?¤َõ(÷?œ1Þd¤?í/àÕf¢?¯ÕÒà®@ë?¶€ùTÏò?¯ÕÒà®@ê3FGL J0808.2-0751@l¡qÿ÷œ"@*Vì¡~jiÀ7/¬ÎÞÀ:¨Æ¨Æ]G?üˆ—'ÃÊ@«i«kG?þÕ¨%xŠ€¿Ý7I²~¿áå=î¿âuì¶wò¿æX|v{ºêAGNfsrqPKS 0805-07?ïðîNÀÎ?aV@Qû ?^#÷b~d}?aV@Qû ?ïßÁÃßÚ?{ùèÝßîÉ?p~s?{ùèÝßîÇ?íº"~ÐÂR?£'±*6?²+d	yín?£'±*6?ïÿ©8£PY?¾ˆê&_?±×+éܒ?¾ˆê%:3FGL J0809.5+4045@fzX`f@?ŠüAÿÀ:-Ÿw),IÀ;Ò½M#Ÿ¿ðÂ^18²#@Ô¾È}1Ú@3
ŸÐÀL¿åŸ"úÚbs¿éz§ä5E¿àF…8ʲý¿ïþ÷b³º"AGNfsrqS4 0805+41?ïÿ)݋ý?«ô¥,çx?µˆ!«?«ô¥,ç
?ïÇÁ'Ëww?'‡LF`¦$?|7DE†?'‡LF`¦$?ïǘ²³Žñ?zI'Ÿ.½í?|3¦¦8†ƒ?zI'Ÿ.½ç?ïù0­›Íé?LÛ:sçÇ?K=IÈb^?LÛ:sçÌ3FGL J0809.5+5342@d' 6m@@wÂ`b@gÀ9ì¿G©ýÀ;èÊõ\8?ÀµÿÅêÓ@ð›äøg°@A)Þ팿ßC߉¤X¿å÷Ù<5ª ¿èßÓr-nù¿Û¥Æ]ÇÜMAGNfsrq87GB 080551.6+535010?ïþ4òC>t?4(DÈ]?,°ÛÌÍ
?4(DÈc?ïÉO;ìù<?"›ºV§G?{Xb	ƒa[?"›ºV§G?ï!2M|Ì?•»ÍQï?›Ù¯ÖPfZ?•»ÍQï?ïßÉÕ?Õ(?eé'ëШ?p`lL?eé'ëП3FGL J0809.6+3456@gNà @À@>Y³¿µÀ: ¿ž(uÀ;›]np $?˜³âèdzJ@Ñ$—'?ú´WÀ±5˜¿Á½~r™?ï ú!Ô
àäíç
¿á©²;&ÉAGNbllB2 0806+35?ïÜq¤J?xà­NªU—?qõÇ-ÚôÖ?xà­NªUš?\fyò?'ª…'ÂYÌ?Ž(æaƒJ?'ª…'ÂYÌ?ïIo1Øá?Xñnwk?–ÒÄýÄ?Xñnwk?ïj(lBçý?'ke¡BŒ/?'ºòw£[?'ke¡BŒ.3FGL J0809.8+5218@dÈ,ÿ§ël@@tw_²íþÀ7¦&áìÂÀ:É×5Ü[?ÀåRÓµ@¼ãÊ?SÓ?þ‡ ›+¿á"P$c?H¿Û@°ÛeÒÿ¿ÛÊ¢Ú¤Àƒ¿Ø	ŸÚÌAGNbll1ES 0806+524?ïþH‡ÈÊ?1ä%Z.?+~׃soo?1ä%ZC?ïÕ5°P4?·÷¦}–I?ue'õ×å?·÷¦}–J?ïÃüÐ>—'?€÷ó	Nó?~—à´6í?€÷ó	Nó?ïÿäJžÿs>ñ¥—´½¿>ëµaP>ñ¥—´¼¼3FGL J0811.2-7529@rtÿ†]}À5n -1'À8H°?)áÀ;hþÇÜ¿¢Pä®qÁ.@t]%ÊêÊ?ÿ* Htä¿ßÌwgjX¿ß¿Ùwˆ«=¿Üб€7•¿ßæ.<îAGNbllPMN J0810-7530?ï®cjÛw?ŠÑYûs?"g%yÉ"7?ŠÑYûs?ïGږéªü?¢}–Ï^$?—­"Ê u?¢}–Ï^$?î­w‹Tù0?šo¸ÙÈU?¥(‡J°l÷?šo¸ÙÈS?î»S•vs?›pÔñ ñ?¤NZƨ˜Ï?›pÔñ ñ3FGL J0811.3+0146@k–gk*@2Ž³ÀŒLªÀ8NâWxŒÚÀ;6~	ñŠ?æaž39ñÇ@HUñ¤ª@D¿Æ©ó¿Þ‰ÚÈ/|¿ã¬Þâ貿àÚWí¢'¿åÿa"<AGNbllOJ 014?ïÿ·òû!?Œõ2ŋ?é ›¾ÿ?Œõ2ŋê?ïÖ7@(ð"?Íέ²?tä_뇽Ü?Íέ°?連ΜÏè?'c:<yË?†YLXÌÊ?'c:<yÏ?ïìD­eÃo?YMBöî`l?c»Rš<'?YMBöî`o3FGL J0812.0+0237@k¢ ¼8*@3=`³žþÀ:þ?5ŸõÀ;'ÕÝÀ¢"^#Í@€èÏa҃?û"éž¿ž;¿äGzr.h¿ásà¸ù"¿Ôê~DdÅ
¿Ã—
f>AGNbllPMN J0811+0237?ïÿ8Ž,÷*?N°ò+è˜?î:a¬ð?N°ò+çò?ïãÃq¬'?x4Õ^?l<ŽSëm?x4Õ^?ïÛuì€CÂ?qkÌ¿é¸ø?rE	¿Þ]?qkÌ¿é¸÷?ïÿÿñC<ß>~±‰nWå9>]y†CÍ
˜>~±‰nWîŽ3FGL J0812.9+5555@d> öð@@ºö€$}ŽÀ:3b-À<¦J'R¿²©É{TLB@Œ¥{úø@ã; 2¿â´®<œq¿ä'§n™e¿ââ~=%X¿× N+S=AGNbllNVSS J081251+555422?ïúÊMîuÀ?Pìa~äHÃ?DÖÈF(ÿ†?Pìa~äHÀ?ïyËqßk,?–1»‡?Æ'Äš"?–1»‡?ï'ñd·Ê÷?‡÷á}™?‹ƒ¦Ò
AÀ?‡÷á}?ïA"œÕ[h?ŽË-\vÊ?—ÏleT'ê?ŽË-\vË3FGL J0813.3+6509@bÝß֔Í@@€0`À:Ž'‰ÚßµÀ;Ô¨·CΌ?ϛXŒÍ@
R¢Æ>_@'°?£Y¿ë	G¨'¿Ûw­ÕL¿á:,‡Ù¿èÀ—Ë@ä)AGNbcuGB6 J0812+6508?ï®ÛÃî
?‹I'ËŒê?"Iyýr?‹I'ËŒê?îë6-͝]?£jÓ$–uP?¡L#&*,?£jÓ$–uP?îG¹tfå?¢ÂhëßÎ?«"h¹'®,?¢ÂhëßÍ?íq'9_!«?¤rNAÔݵ?´vÆ5òª?¤rNAÔݶ3FGL J0814.1-1012@lütÿ†]}@*m{Ÿ³À8ú"mRÀ;L†ŽúÚ&?Åzm]À>c@K9Ž—@'8`Är¿åÚîÄÕmÁ¿ä˜¢dT¤ƒ¿Û+z	ää¿àDžt¨QAGNbllNVSS J081411-101208?ïÿDæ¾PX?4H6ãß+?c(5ôî?4H6ãß?ïÑ5e)Œ?íp½Ä­?weMkp9Ñ?íp½Ä¯?ïØ-KyÕ>?|̵ƒìb?séZCaN?|̵ƒìb?ï×õnžÄ?e££±e?tH°õ¹?e££±j3FGL J0814.5+2943@h£3v@>€'ÍÀ:y¼>§À;ëtZÏY?㪛u(@
O
–<?ÿ¦à©ùc¿îí(ށ¼>?èŽR€«a¿àÜbSS±z¿å÷/"ÃAGNbllEXO 0811.2+2949?ïd''áÉû?—.mŸÒÕ?"o­ÃÆÀÊ?—.mŸÒÕ?éËTXû?ȔMϝ-n?Ë°Ò¯¢œ?ȔMϝ-m?ï±b?"L
dQ
?ŸiÜÜS¯?"L
dQ
?äþË¥wdí?Á	Bfu5ÿ?Öhµ6%?Á	Bfu5ÿ3FGL J0814.7+6428@böW´@@›aßîèÀ8Žõs}¦À;}ЍK­}ÀٔPXÞ@ú­ê^ƒ@_û¿~…—¿â{fôîC¿æüN^v¿à¯±íè@¿ãNŀ'W³AGNbllGB6 J0814+6431?ïÿםä·>îûŒ2=†6>ô1}¤ '>îûŒ2=…g?ïÕr¶wßz?€šÿƒÝ]?uF¤ÄC*?€šÿƒÝ]?ïì^Çk"ë?eòûîΣ$?c¡8"{£?eòûîΣ.?ïÿûàDK>ÌÒH$ã¢>À~íÂÓ>ÌÒH$ã#¥3FGL J0816.4-1311@mYb¯È°@(AŸ˜À8cKB±ÂÀ:ßÄ"ïï?èÝÌ.A[ë@ß²ì¦ÜÎ?üméµí¸?hA¿µY‹¿áÔ'€]Ē¿ËyÓ
D¦¿ÛL'æ>ZPAGNbllPMN J0816-1311?ïü´SÚ¬?<¸nÿe«?:]a*Ÿ¯4?<¸nÿeŸ?ïÆØÓô?ˆFr.s'&?|ñ–œ?ˆFr.s''?ï¦(íåt?…œøê÷?†uÛĆ¢ä?…œøêô?ïz$ü»Pá?ô´²-Š?»`h•ãÜ?ô´²-‰3FGL J0816.5+2049@iMfŸê%@;¦1_ô\^À:™8I©"À;ï"öW
?ÈJ]*lT@
ž‡½N)¯@?è`&0k?¸2Çä–Ô)¿Ûv<lí¿¿Ùì£{^‰è¿éf"6Þ'AGNbllSDSS J081649.78+205106.4?큘¿X?·Ñ¼´X&?³ó:¥?K?·Ñ¼´X&?ï*oVçž?žLŸ¯¶?š¼²#7?žLŸ¯¶?ëÓhÅø'?±s"Þi"?À²_ôè¶?±s"Þi"?îa¨""?™:ßZO?©åw.·Í?™:ßZO3FGL J0816.7-2421@nŠÀ€ù£@ïÝëÙÀ9HÏmýÀ;ohی¿­r†fSJ@Pkþ*é@thŸÑ—¿àf¾ ȳŸ¿ç¾o+ÜÒ©¿è^Ξw銿ÛîÂôdtAGNbcuPMN J0816-2421?ïýÓ[¬Š‰?6"§å…Ò?1e"›«¾«?6"§å…À?ïý¹Pm$?''}ìe??~!#WÉn<?''}ìe??ï3¯TÌ?"*p;ëöB?™ŠfŸø?"*p;ëöC?ïð£áù?UJX&6L*?^¸<
÷á|?UJX&6L&3FGL J0816.7+5739@cû;@³Nw@@øÍ?¹SsÀ9¦Üx;{À;¡iÀŽ¿çð+‰y@mJ
jKÎ@ç@ó¿ãýæzÕé¿àǵ…Õ¹Ó¿ÙÖ͂»lä¿çj…QãøbAGNbllSBS 0812+578?ïý<Kù ?9£ßOOl?6} 3^?9£ßOO‡?ï¾ÞÊpà­?…$*G±™?€HMcÇÔä?…$*G±—?Hqšñ?'õõ!`ïJ?€Õã™C¿ï?'õõ!`ïM?ïñÖ:EMÁ?[®Œ¦Õ?\S‹ud{ë?[®Œ¦×3FGL J0817.8-0935@lúš?Ffí@,¢9 4¾NÀ8ß¾®&˜À;G²3ÄR«?笃›‰ù@ŒO¥¯§x@YIàsÈ¥?§t¹f#Ý¿Þ7Áá
,¿á3צx,ë¿àï›þ< 3AGNbllTXS 0815-094??¼øÖ?…{ÒéF?ˆÔ0Áʘ?…{ÒéF?îÁZu¼'?®ï–+Ÿq?£êX®46å?®ï–+Ÿr?íà·¦gúS? ?ôõˆ×[?°úBÌÀ-k? ?ôõˆ×Z?émLsüò?¯/, ?ÊJÎ05‰?¯/, 3FGL J0818.2+4223@fFˆ?Õ%@@³YLVÀ7a{E¼À:Ú;2Ûõ_?öÞÙ|ˆ'´@›:Ö@?ÿŠx»}š¿ß 0öܯˆ¿á~ñ`°+¿á"t˜¼¿¿æëÓ=)V;AGNbllS4 0814+42?ïô#žÔD?YijV'w/?WѸÂWwµ?YijV'w&?ï†5L¥î?"¾¬¨Kçä?Žr¬Ö¼D¦?"¾¬¨Kçä?îä°l{E˜?˜D••¦þ?¡´ù8K¦~?˜D••¦ÿ?íӏâ+Æ? ¬ƒ¬\0?±c€î¡Ï ? ¬ƒ¬\03FGL J0818.8+2751@h_™÷L@>e;?q/À:30'8'À;ã:ÆG¿ÝS!@	«l'¥^Ÿ@´Þ?ä"¿ãÕgš1Þ¹¿èÓ÷4¬Û¿×ö´·Ø¿ïÿÙÍ|[AGNbll5C 07.119?ïéYe¦?‡éÂí°W ?f¦š~Yc‹?‡éÂí°W ?å¡ï´.Vå?ӛfì–_?Ô¼ —£R6?ӛfì–_?îdÔ'é¬? ´ÿ@A?©²½nu7? ´ÿ@A?ìŽûfW°?µŠŒïRB?¿sˆ$ÍB~?µŠŒïRB3FGL J0820.4+3640@g Á¿½ð'@@pÀOæÈÀ:³Ô®BžÀ;ã·N¶Fy¿ø~&¡l@Ž£?µ¢@Cà{Ö:¿Ü:®%•¿çk	¶©û¿âÑbk/#¿àIq	úÍAGNbllMG2 J082018+3640?ïù8"úO?T\¢ 
ý?KtÆÁ?T\¢ ?ïÓ_¨Vq?€êr"Š(?vP+ÔÇ~œ?€êr"Š*?îÖ¼Q·Ç?YhόY?¢":䎋?Yhό\?ïý6ÓÓòÇ?9qƒ˜ë|?6Ia`iÊ!?9qƒ˜ë{ê3FGL J0820.9-1258@mfbŸœèÙ@*SŒÿWc"À:w "@ºÀ;·+rt'¢¿òzí¿`¨Œ@€â¦Rå€@,Ó P—ó¿êâ=‹Ä¿ây'vg¿ÜõF""ð¦¿æh¾òæß?AGNbllPKS 0818-128?ïôZ†#^?\çÌÚ©-?WJó¹ÍCã?\çÌÚ©-?ïÝ$Ž}b+?z‰‰"0?qm¸ÁNë?z‰‰"0?ï)
.b֙?•™[9ƒÑ?šÞZ3¥-?•™[9ƒÐ?ïú®sÇTò?IœP®F<?EF0â¬6z?IœP®FG3FGL J0822.6-4250e@pE•:À
5ðŸºÅäÀ7A9†3‹À:H{$cŒ—?ñÏoÏpÁ@}3¤GG'@iº?V'¿ÉŽ;l'¥¿ã3݆Xt¿ßŠRiY_î¿âýŠoZ*ïOTHERSNRPuppis A?Øÿ;Ù"1}?ÏBoëdo?ã€bnçB?ÏBoëdn?Ñó–´0d?Ñ|ä"*çr?ç4¥çÍø?Ñ|ä"*çr?ä,U;j?¸©5|7q?קUù‰Ç)?¸©5|7p?ÔsáIK»{?»öB?åÆ[Z"C?»öA3FGL J0822.9+4041@fŒ8¾øγ@A`	UÀ9Ê";ÝÀ;¯ÌÐþŠµ¿ß®Õ'[°ø@©F>RÌ@éà‰¿ä—ìëÑì¿å¾Ó¨'·¬¿êîCe'¿ÑÌÎû%OÆAGNfsrqB3 0819+408?ïÿ7_ß«(?$'«8‡Ÿ?
šþQ?$'«8‡…?ïÙêÑÛ?}óIhm€?s
—p'M?}óIhm€?ïҜÍ=–?t1Uê	J?v±ø™a55?t1Uê	T?ïûÍB
?@x;ö{¦»?C"ËÎ÷ɜ?@x;ö{¦µ3FGL J0824.1+2434@hàéߗª¬@>Šô PmÀ9Í]®1À;¬'Ä"Bh¿®U;¾˜Û@I¯K‡"@$e –"—¿änǬZ/¿ç	®éî¿å—÷9v²ÿ¿å°¾Õ˜AGNfsrqB2 0821+24?ïý@W»t?7æežw@0?5ýC'$c¤?7æežw@-?ï¹´*W?‡¿™_©™?¸õj=(?‡¿™_©—?ïÎÊî´:°?v²¬kÇñç?xšˆ¥â§Ã?v²¬kÇñÞ?ï±ñivö?w$s™2˜?ƒ¾Ã¥¢BÄ?w$s™2—3FGL J0824.9+5551@d?n «†@A'Ÿ¸—ŒÀ98cϳ1À;ÑF2ê8?Á ¸è®@¢é¹íw@ÙÃߓMû¿ã\<´š¿ê^+œ;¿ä²67ìÍÁ¿é—ÐAGNfsrqOJ 535?ïÿŒ?ªÔ?°'x{›?ð{U
?°'x|]?ïÑ'$îUU?'|b6Væ??wlmˆÕUl?'|b6Væ@?ïÉÀ	ºN?|aL†MÖP?{û"ØþÞ?|aL†MÖJ?ïü%p"|T?9Gñ:—r#?>Ô{d]4?9Gñ:—r3FGL J0824.9+3916@fį_Ô{î@AU_­åÀ9Ć4b\À;Õ½5?âm¸¼Êv@jŠ'T@>`
ø¿èžŠçq‹¿ÝZ"e'¿è(ð@¼«¿ïÿà­Õ:ÚAGNfsrq4C +39.23?ïcñ™ªì5?˜rø+¤s?"ÌÊ¢y ?˜rø+¤s?íÅ
UÍÒ?±"ÏìŒzU?±×•WA'u?±"ÏìŒzU?ëuzEß#š?­gª®~$=?Â*èƒq™?­gª®~$=?ë­ÀÙc Õ?¬ûøHKˆ?ÁHüšs|¬?¬ûøHKˆ3FGL J0825.4-0213@lFÔà—"ì@3®Û@-¹À:S¤A"HGÀ;Ïçû&|l¿¸Åb$Lm@	2Á濽@5œŸ]}ß¿ç\ÄfZ6¿ä7;‰ªˆ¿æpÇNaÖ¿æƉ"ßgÑAGNbcuPMN J0825-0204?ïåeÉ$ø?h ëû´+C?jšð6Ûz?h ëû´+E?ì:¸°Z?ÂþwùB?¾*?j}/@?ÂþwùB?7X)?˜É·f%L?¦eŠw-X?˜É·f%M?瀆>ï}ô?½±Ó£<?Ðþó'!?½±Ó£<3FGL J0825.8-3217@o"Àh¡@
i¿ÿ´ÖŒÀ9d8Ž¼ÇÀ;Z|¼A%¿ýÿÈØK†@{ âù‰ï@ê®YÒY¿çq¼*	¶/¿äó®é¿ä§Úb{d¿êk…xêAGNbcuPKS 0823-321?ïû®µlN?DTòƒœšª?AE*O¦À¤?DTòƒœšˆ?ïё†ß q?‹Âjp=àP?w7</Ç?‹Âjp=àP?îŒÉ)Ú?œ{
ÖQ§Z?§3nb`
?œ{
ÖQ§Z?ïÿý{"‹O>Ç	Œ4 ƒ>´#c¥‡­>Ç	Œ4 >z3FGL J0825.9-2230@n~à°¯`@!Ùäúœ>À7ŸA¥ÃtÀ:Èï'j¨?çÏ™à@4%죬Ã@cÀCÒh¿Û‡y§Çëοâè$Zìú¿ÞíñN{'¿Ý>"[U!AGNbllPKS 0823-223?ïý›á†¶ô?2#_4ŠŸ¡?3 óÊH^;?2#_4ŠŸÅ?ï¥UÉÕò?•.Uqt?†ªŠƒ\¾?•.Uqt?ï"­r2? ¦Ñ}ó7?Œ7T£s_±? ¦Ñ}ó4?ïzQ~1.b?"ÙHÎz²?µÐ9Ú3æ?"ÙHÎz²3FGL J0826.0+0307@k¨ø -à@6mÀÊ`À9Ýa…V¶À;¬½D¦"¿ìïAïíö@ 2)gW@<Çÿ]˜·¿äàÿÆì…q¿áT'8§;n¿×ô'ª,¿ã)ç/#¯AGNbllPKS 0823+033?ïÿc>!§Æ?mo'–Z¾?˜;Ë?Ø?mo'–[ÿ?ïÜö½áy‰?|2—Dz?q"¡C;ß?|2—Dy?ïæGCé&?p§N+ùn?i¸¼âÙÐ?p§N+ùh?ïýhšdÛù?39™Yù·¸?4»,Ù 6û?39™Yù·½3FGL J0827.2-0711@lޛ6†¥@1Š	cr–À9ë:^ ŸGÀ;²ÔG'‡¿	äÐçž@
j°ëoÐ@‰žŸgäÁ¿ÞÔl´Z¿è~{å˜d¿ÎƒÉÈò‰¿ÙD÷}$™AGNbcuPMN J0827-0708?ïûX©‰=Î?Eôrßt:ò?BYÛÆ7?Eôrßt:ô?ïÐC"SgS?€ǾÖ?wÞ6VLW)?€ǾØ?ï™l7:ðï?"'`Ãï—i?‰¤ò1CÄ??"'`Ãï—k?ᅪ_é?tLxâ…ì?€º¨Å®?tLxâ…ð3FGL J0828.5+5217@dʽQï·@Aã(CìÀ:ÊÐþŠ´úÀ<!‰X¿ºáӞf÷ @g¤Ôá@'¿ãZX¿ëê)1°.å¿Ö6¯¿ÔOÙìðڿ당Šá×AGNfsrqTXS 0824+524?出Zú¬?ÒÁيw[T?Ôð‹J
§û?ÒÁيw[U?ìƒÐà0Ý%?¿«ÒG՚?»áxþyâ?¿«ÒG՚?è"_"Ózl?ÁÍqy¥´?Ͳƒt²P?ÁÍqy¥³?í˜ÜýfN?«¶r]_ž?³9Ï]‡?«¶r]_ž3FGL J0828.8-2420@n¼WÀ±5˜@ Õ¶`#× À:6ÄíÛ:NÀ;±Ø{V¸¿æP˜#Lá/@
Ū‰€ò¯?ÿþ½?'‡¿ÒLS'ÿ¿é×:$ȿȏcüï2¿ãˆŒ£^aAGNbcuNVSS J082841-241850?ïþ¤p"•à?&Ɉ´³?%¸÷¶¢¼?&Ɉ´³ ?ïÇ©õFww?ŽêS%?|+\ÄE?ŽêS%?ï²
Az¥1?~˜éŸß€?ƒ|¯¡V³¥?~˜éŸß‰?ïøsñ‡ÍÏ?MÒY~ˆ	Ô?N09àÈŎ?MÒY~ˆ	¿3FGL J0829.3+0901@jý؈v\@9ÓÉ¿Ò‡À:¨L…ЗÀ;à\KZqf?Þv~;U}@c‡'ÛåD?ÿ(ÜP'`¿ïÿÕYu?ïýv8t^¿àò±C÷.¿Ô÷P0;~~AGNfsrqTXS 0826+091?ïìnÎTFŠ?_ž·l:÷?c'1«¹uÜ?_ž·l:ø?î ÒhK?·('"±´?­òÙ{Oç?·('"±´?ïY"«K­?Š´hd/æ?"ßïj–ŠO?Š´hd/ì?鏓…¼¸a?¾gf¾"–?ÉÁ±é
{?¾gf¾"–3FGL J0829.6-1137@mf[ ¥&–@/\7 þ}IÀ:SÐ-hïÀ;¿ŸàÛwŠ¿õb ¼8*@AåÀ8À?þ;Úß_ ¢¿Ê±¡NU	¿ìF»,Þ§¸?Ñ~°ŸšŽ¿Ôr¨©ïAGNbcuNVSS J082939-114103?ïÿ~'ò…?ÙB™6¯Ì?/¡¼ïvF?ÙB™6¯?ïâ{òÖz9?x?´L$Ä?m"
)…ÇÁ?x?´L$À?ï´&(ü‡°?€µGÖP"/?'öuÀÞ?€µGÖP"4?ïÿõ`Á>Ý0}ª&¯>Õ?è}ñï>Ý0}ª3FGL J0830.3-5855@q%ˆ¿Â"OÀ&ã
F:À9Z¾ÝöÀ¼À;†aQS°?è3ˆ2˜ü@=òFƒòé@Ý»à~í¿è˜p&Œ9¿è¬-ÎFl¿äÌ~?Ã\¿ïÿ¯í1àçAGNbcuPMN J0829-5856?ïì
}Íùœ?jÁq'fÌd?cò'2c?jÁq'fÌc?èÀM™QhÌ?ʊm˜°¹?Ìþɚº\Í?ʊm˜°¹?îòfiU˜?–Ò¢Q§? Ùž™j¦v?–Ò¢Q©?èé­Ù|ˆÛ?¯ú=Gì¶É?ÌYHš
ܕ?¯ú=Gì¶Ê3FGL J0830.7+2408@iòà\̊@?Ô· "À8¯â*ðoÀ;'çf¬"?î,Û`–÷1@è]…TÖ@í?³õ¿å@É-}^¿é6ÀNí¿çr
²©`¿ìm«ÞöAGNFSRQOJ 248?ïõ€¿ëël?SÊᐡº?Tþ€()*¶?SÊᐡÁ?ï…;E!~?'®Ïß
‡?Ž±.·œ C?'®Ïß
‡?ïIóL3½`?'s_B"??–Á–yˆSâ?'s_B"<?íìËؙ•R?žKŸ\UÁ–?°™¡;3Uy?žKŸ\UÁ"3FGL J0831.9+0430@k–Š r~@8^'ŸªTÓÀ8&–5À;9¯4^¬?ö wÔÍÍ(@*íEé]@°Ì`Á5ë¿Ú~Oû"´õ¿å
‡òÓ¿ä2z ë¿çC^ˬ*/AGNbllPKS 0829+046?ïüø'(æ?6.ß·o¢?8>ƸÏT±?6.ß·o¢^?ïÒ¦ew9§?VÿHéHN?v¬ÍDc,Î?VÿHéHN?ïc4u¸?—M€å—a?Ÿ"™qI?—M€å—a?ïåཥ‹?dù+±ÄÕõ?jíBZu‡?dù+±ÄÕò3FGL J0832.6+4914@eC[ÿW~@B6| À:¥kÏ[óFÀ<>ô1•¤¿ÑHe²¿ãä@
'žÜsß@è? ©Ù-¿ºä¸·þÝ¿é+'Ÿëñ¿àöäð§j¿çJ+í;#ºAGNbllOJ 448?ïò"spy:?fÇ´ƒO0?ZÙ
Œ?fÇ´ƒO-?{:×?—tRæTdæ?‹Uá1J:Ù?—tRæTdæ?î¤óô‰?€]ؤˆ	?¥¾ž À·t?€]ؤˆ
?ï¤j²'î‹?}']"i?†åS[D]M?}']"i3FGL J0834.1+4223@fSëßL+R@B'±ÀoÀ9f:¢"=_À;Ȍ{£åM¿ôž6ìü=@<¦Ú'Q@ƒÀ`óJ¿å«cÛi8¿ç©Á‰Å©¿ÝTPф~¿é£Ü^nAGNfsrqOJ 451?ïöû×F*?VÇ÷I?RQçs©ã?VÇ÷I?ï›eAÔò®?"oÌá9Ø?‰&¯ŠÃTš?"oÌá9Ø?ïò½9Ï?–þU{…I?Ÿ¨XÆž?–þU{…K?ïöW˃T?Wøo9»G?SßPhùYZ?Wøo9»A3FGL J0834.7+4403@f^Ñ·@BH{Àj¾»À:l{¯£ÇÀ<Ä3¡<À¨ˆ‹ªB´@%š_'6Ï@½:¿™ˆ}¿ê#"±*ãa¿Ïh
Ô"	H¿ä&\tŽáô¿â7ÁGˆÁAGNbllB3 0831+442?ïøM.-?V~œŽñíæ?OšËGKÒ¹?V~œŽñíà?ï×¢[À ?',©WÚh[?t.Òÿp»?',©WÚhZ?ïV^ێW'?'rÚÚâs?•4$Ž5
Ì?'rÚÚât?ïÿë¡Îê€>óp(K=D>ä^1å	>óp(K=C¯3FGL J0835.3-4510@pxß¿ƒ8.ÀLV ž9À2ˆ©ÀXJDÀ8Çå"S·@衦ˆ›@ø9'rÞÅ?ôž£¼ˆ1¿Ð†bbÔ>¿àÝskâ¿å>¢ÔšS¿ì̋Ç0PSRPSRPSR J0835-4510?#ñ1tãD?$HJ›õä?ïþÀìè¾1?$HJ›õä?#0@Ä;|?B1U@|K?ïþÌþ»ó¾?B1U@|K?'JhÍíí?…†ì"­€%?ï¶Ö\˔I?…†ì"­€*>3ú'ÖI$'>D
Wn!É?ïÿÿý€­Å>D
Wn!É3FGL J0835.4+0930@ko?Rü&@;fi¿·:"À:WozânÀ;Ô$n:¿Â"+l=@³ieIZè@OÉ Gˆ«¿ä'Õ""¿êV_T?·¿Ñ©Îée<x¿ßoò2bAGNbllGB6 J0835+0936?ïû—k;óÞ?GñeÐN]?A¢S0ˆm?GñeÐNz?ïtþ
5j=?œ6"•Ùe?'`>YR¸`?œ6"•Ùd?ïU)˜
?"IlE(]+?•ZÌü^¿¢?"IlE(]'?ïf<ŸûÛ?ŒES8÷âH?"8l€"Ô?ŒES8÷âJ3FGL J0836.3+2143@ih*Á	J,@@$ÓÀíÀ:K/ÉgeÀ;Ô¶JªH¿¥ŸtD¸{8@
†Ã(3P@†š@ˆ†L¿çZþÞdFH¿èð­&¿2¿çÙÔ5ˆ^¿Ó(^öQø¾AGNbcuMG2 J083615+2138?ïþ"ã9dË?)û•©…q<?&±Ìi³FÙ?)û•©…q?ïÌóƒæÙQ?…g#¾Æ?y†>"WË?…g#¾Æ?ïÀä°äU¤?uÔ·ù"?§Õ-?uÔ·ù"?ïìgKbœf?^ÊMK:ÞÒ?c˜´c™Ú?^ÊMK:ÞÐ3FGL J0836.5-2020@nsŸ‡ð$@([qàíìÀ9"ØC""À;¢Þ"umj?Ø[·Êßõ@ - ®@Û$¼"Û¿ècpÎQ宿鞡S!e*¿é ,W™;r¿ïýÁ\‰ÌPAGNfsrqPKS 0834-20?ïãúlÏ1j?n´Ü͌.?l"0Εç?n´Ü͌.?ìTꊲ6@?»±D‹M?½X«ªnMû?»±D‹M?îmE¯I…t?ó	QB?©+¥g¨Ï?ó	QAÿ?çÚXL.ç?³ÖHyb´(?ÐKçOg¢1?³ÖHyb´(3FGL J0838.1-4615@p‹ƒÀ~à±À\ `ˆ+À8$›†ãàÀ9¼n9™~Â?öű:5¥@ï†<š?ÿϾúQ?c¿Ù:E E›¿ã3õƒ¥¿éµŒ©ÇG¿î¥x?V×þOTHERspp?ÏŽIX‰+?Ȳ Þc³?è<\m©Ýµ?Ȳ Þc³?å'z'#?ÒòYu˜?Õ±û
Û»?ÒòYu˜?Ù©€þݐ?¾Ü[óEj?ã+?€'7¹?¾Ü[óEj?Ýd_¢›®?ÆÌ+?UÖ?áwÍÐ.²)?ÆÌ+?UÖ3FGL J0839.1-4739@pžæ?šIÃÀ#Á`]öÀ9¢t3®ƒÀ:ZQU]*?ñò÷c#f@âeæ9@®èŸf7B¿ÞŒ£çÑ5¿í°˜ƒïä)¿ìZ¾b¦¾?Ç¥}=OTHERspp?×öžCƒ#ª?ÎVÄÑB?ä°Þ>n+?ÎVÄÑC?ííkWC?À½ã†6v"?°"¥Eç/Ê?À½ã†6v…?áQE\¤	?¶n®ù]ï?Ý]uG·î?¶n®ù]ï?ípµÆi¸!?·(å\Fp?´zQ̲>÷?·(å\Fp3FGL J0839.5+0102@l!O?Ù3ã@8_L?s³VÀ9È[[piÀ;ďñz+??ò%ëú}·@<'è§HÚ@æ­àMˆ¿ºsçûž¾¿¿à‡Q¿ ¢ô¿äE|	w[¿ïÿ‹Z,$AGNfsrqPKS 0837+012?X	å?©ÃFYµw?¥~֚a™?©ÃFYµw?ï¦Ú1ó¢Â?‹L_¨ú‡?†IsƒO¨?‹L_¨ú‡?äÛTè¿ ?µŸX—žD4?ÖIV.€¿ê?µŸX—žD4?î杽K¨?z‡Ž&]?¡Ÿv$+E~?z‡Ž&\3FGL J0839.6+3538@gcôŸM¡@B>n¿Ñ;ÇÀ:w»"€^À;¾–ä•?ˁâmÈÛ@
íæšÔ,=?þÄl@šúÿÛijãà¿Ø)ÉMˆÁ¿Û§7á\•œ¿ã°UþdIAGNbllFIRST J083943.3+354001?ïÖ®6b/?uˆj{\7n?t¨òäÎçÅ?uˆj{\7p?ï06Ÿ]? í5"õÊ?Ÿ¹ù,š? í5"õÊ?ï+icûwß?'›¨7\UJ?š'Ó€'÷?'›¨7\UH?î>ž?škØjl?¬~æ‰?škØjl3FGL J0839.6+1803@ióÿ`Ï‰@?ÁúàŽµÀ:g8Yã¡%À;Û²ìPö"¿ñ~n¸Œ@WÕé4-?þwæ Zé[?µ&Pƒ{H¿ß3pÍ?ð¿Ûÿ)w-ð¿±bÓkÄÁˆAGNbllTXS 0836+182?ïø†k±#‡?SŽ®ÊÃó¥?MæQ;qáþ?SŽ®ÊÃó¥?ïÛK±,*?ëXaDF?rZ'tië"?ëXaDF?ïjLÈãÖ?MªŽ?'¶fãÅ?MªŽ
?ïÿeÁw¹?¸ÄÈD¿?_‡ÑÙÐ?¸ÄÈD.3FGL J0840.8+1315@j›Ÿ˜·@>+?8$4À9¢Àøƒ3ýÀ;À
éh?ëz¿Ôäì@9Ua0r@¾Í­ð>¿â5JBï>¿èy$ÞÔÿⴛ<Ú«¿ïÿ¸ÕҍŠAGNssrq3C 207?ïÿ$<ZB?)8öý‹•¦?x|T· Ø?)8öý‹•ú?ï;™ëz?'›*ψZé?ŒÂ¼*?'›*ψZê?ïL¢¸
¿;?'`Ž΋?–k¨þ¨À?'`ŽΊ?î¤pæû?"h~iv?¥¸ÿ¡žpU?"h~iv3FGL J0841.3-3554@p
Ձ¥‡@
æ1ÀAyÀ8 TS>kvÀ:ðÓu]z/?òã(­"÷@tpȕ?ü:¿ë½Ô¿×¿¿¸èz¿Ö'´ƒ]v¿Ê`P¶6¿ÜòàèbªoAGNbcuNVSS J084121-355506?ï÷9z…kÆ?`9¿?‹¢?Q
õ(u?`9¿?‹™?ïj"ÿ!w?²ws—ç?žò» Ñ$?²ws—ç?îë÷Yؓ?—…UXEÁ?¡@ŠbvΚ?—…UXEÀ?î_ð‹Ôg%?šÿ×R·?ª÷B¹¼?šÿ×R·3FGL J0841.4+7053@añ'à@A7E AYÀ8	³;+O9À;€æàtI~?ûÈ=ägF@i•šÜe@<ѯµÄ¿æ›BŒÓŸ¿ëŸÏW…g¿ëƏ¨Ì^à¿ëÆl:]@oAGNFSRQS5 0836+71?ï÷D¾•ðÛ?PÈ¿MQ?Qv'ÔI?PÈ¿MS?ïÏƶèñ?ƒŸî´²ú?x¤±‡Ç?ƒŸî´²ù?í!êTŒhÒ?¦
öŒÉ?¶ð­[œ¹t?¦
öŒÉ?ïüõ™Ì÷á?>R2ÖC"T?8S1˜@ô‰?>R2ÖC"m3FGL J0842.0-6055@qN9¿ß~€À&Ð[À6ãÀ9	füŽ[xÀ;z³Z4ÿ¼?ñ0èóžó¡@¾Ù>Js@ŸÑÀ§zƒ¿ã'»¢Fֿ嵊ÂÕìË¿àé4ü®^D¿í#ÞùÂqAGNbcuPMN J0842-6053?ï¡7e›Ú?†2¸b4¸4?‡¾r&™	T?†2¸b4¸4?ç¨xîùrB?Í?˞ƒ¤?Я"
|?Í?˞ƒ¤?ìÔ¾'o?ª"p~kÇH?¿AZÇÜv?ª"p~kÇH?é;£†¨,?®Î×Ö2?Ëqå_¿Q?®Î×Ö23FGL J0843.1-4546@pÏ`Z³«À{=ŸrÌ{À8¶Ôš÷g«À9ïg ù	l¿òŸXj¥:b@Í­ð>@D5¿æ+Å`qÚ¹¿é8"ѳ¼[¿ét5A*l»¿ÝrFnyZOTHERspp?⭇'ÈTü?Л/"°?Ú¤ðÜoV?Л/"°?ïÆÀ2.%?³³¡ÝÊ?Ÿ§'ùº;R?³³¡ÝÊ?â'}WûBN?¸BÂ
,¹X?ÚÝP	{f?¸BÂ
,¹X?ïüTmçíM?JrÍ µ)?=\À•˜I?JrÍ µ23FGL J0843.9+5311@d¢KZS3@CÒ_³Ä¾À:è>BZîÀ<‡ªƒÍ?¥sÀìa@UÍÕ
ˆð@ëõƒ¥¿æM¤_è•M¿ã‡:]N*¿Ú åÓ¾
¿ïÿ<!H"AGNbllNVSS J084411+531250?íƜFö	>?µ²'ÖÜì?±ËÈO¶?µ²'ÖÜë?æî°0EF?Î@$|à¿?Ò"ŸŸýuu?Î@$|à¿?êMo‡'?¸äñÄNè?ÆÊAáÃѵ?¸äñÄNç?ìp<¢ð^Ä?®D<
?¼~è}	Ý?®D<3FGL J0845.1-5458@qT@(äüÀéá€8ªÀ8µ|N/8À;G^X?éˆu¥@X8ü÷@[=ŸrÌ{¿ávý¨À[®¿å»ÒÿŒ¿á€o$Ç8¿éñd—ëTÞAGNbcuPMN J0845-5458?ãÇ£Õ"QÊ?ÇCô›\I?Øp¸U»\k?ÇCô›\I?­ÎÚîîu?ºXŽQ¶ó?î#"Q?ºXŽQ¶ò?äe­Øwœ.?·¹ìVõž?×4¤OÇ¥?·¹ìVõ?ЉXُ?°ÕŸ`·(?çó»rӓ9?°ÕŸ`·(3FGL J0846.7-0651@m,xßzN{@5Φ ™@À:©-‹S†À;Ãý…Ò<x¿‹GÿFô+@	 ¼c1@Ò[ßú¦û¿ävÿ¨r¿çêIf~u¿ç"Öì‹Y¿ïûõ-Wë¾AGNbllTXS 0845-068?ïê"¾®ÿ?eqΝBê?eðkAQ7?eqΝBí?î<}uALí?¬4œò·"j?¬8(«ë13?¬4œò·"j?ï®ø'H?'áÎÙCW­?
>ï·?'áÎÙCW«?ìþ}Š 8i?¦´±]·ò/?¸ªþ<À?¦´±]·ò/3FGL J0846.9-2336@nøeÿ£¹®@(i'¿°"˜À9	åQþÐUÀ;VZU¶ëº¿ä@$ýTBç@¯ôüåš@6ãtt¿â@")N>¿àö¸dq)õ¿ãÅ1˜±ð±¿·eÖÞôl¤AGNbllPMN J0847-2337?ïú[A<´?F"µŸ°'?F"¶û
.ê?F"µŸ°ö?ïݕgÂ^?{P¾èuâ?q5LÐü'?{P¾èuå?ïrGš»?Ž%âÀSi#?'·l¨Ï?Ž%âÀSi!?ïùÿÙµ?F3‰;Ö#?HŒ™+ñm?F3‰;Ö+3FGL J0847.1+1134@jî4 ½@>à•¿ðExÀ9¾Ñk—þÀ;x}›ö¿î|"eÞ^Î@oS"ºd?û؅_¥×ë?ïÍå=Sj¿Øg½¯ß']¿×ÑåÙkÊ1¿Ð'oO²ß€AGNbllRX J0847.1+1133?ï÷)Z·_?R,¬ÇªÁÕ?Q­J'@É`?R,¬ÇªÁß?ïÚršù+Ö?}})žãÝP?rƲƒj'?}})žãÝQ?ïxmRC‹k?†j»±_Bï?òU·Ž'«?†j»±_Bï?ïüoÑöŒs?<šX•O?<pKœið?<šX•i3FGL J0849.1+6607@bY_í¦a@B8y@]¾!À9Ô"Nßa$À;ØgÕÒ/?ÄíSÜ\H@ä'áqI™@!ŸàZž¿Ú)ÙuÛ,¿á™ ù;Ò¿Ò"¦wgYo¿çáMž™AGNbllGB6 J0848+6605?ïô¸ .?h^©î±|?VÈ¿Ï£
?h^©î±~?ï©­ª±?‡ÉŠAÔß?…"¹UxSŠ?‡ÉŠAÔß?ïj'°¼v8?.ÎIø?'­©èq8þ?.ÎIø?著{–;?{NÕ¶ž?…˜!:ZqK?{NÕ¶œ3FGL J0849.3+0458@kÏÿšÏú@<hÿƒ~À9Ùé¿KÛÀ;£Ö™Õ(¼¿Ì¬s"é@CŒxsÚ?ÿƒ3Ù'?ïÙ]KW
пãCUˆPN«¿ÚJ,Qº¿Ý]4wð–DAGNbllTXS 0846+051?ïðéq0.?eM¸ú/¿g?^-Ÿ£‡?eM¸ú/¿i?ïºÏšð.?jº½vYF?LCü4?jº½vYG?ïjô|°t.?‹\+)€—?'¡piñz7?‹\+)€—?ïµR½û ?̯õ"«j?'«y7Æ?̯õ"«l3FGL J0849.5-2912@o"
ŸS @"vï`¥bÀ9†°>÷Œ"À;":]Éß³?ÙÉü	È£@-Æ	99²@ñ¿€3-¿âw"©Կ㆖O7JÅ¿Ö֙qM¬¿åÿ¥2AGNbcuNVSS J084922-291149?ïèJú·+?i"—'Š÷‹?gµHðÔY?i"—'Š÷ˆ?ï Úܤÿ?ª*°j¸­?›ä¤k`?ª*°j¸®?ïjýešã"?z"í¡ÜÝ?' SL£›Ý?z"í¡ÜÞ?îõ¡oˆ¾?–œ2,¶?®¥ét2?–œ2,¶3FGL J0849.9-3540@pTÀ%@ùJŸ¶i3À8ýJh˜À;9©y
­Ù?äϳ?'@äSV>P@÷«ßla¨¿ã߃<yDZ¿áаd6`d¿èÌÕ÷vw3¿å%¡8/­~AGNbcuPMN J0849-3541?ïçs°½ú(?ioŽªºš¹?hŒOBØ[?ioŽªºš¶?ï¬(˜Ñ´C?"ÈʑœWM?"õÙ˒ï%?"ÈʑœWM?înËFºq?˜*'×6²Ú?©ƒK"Xù?˜*'×6²Ü?ïÊ0·P«˜?oï[…‡¥?zç¤Wª4m?oï[…‡¡3FGL J0849.9+5108@dóM@$³>@C‹ßœ³*À8…JÿÓ?À;"2¨É¸E?ð;çҌªH@'øyxçÈ@Bsàwy‰¿áJÈ|ÊÅ¥¿ä"W¿â+}Aý®õ¿ìéº~wAGNNLSY1SBS 0846+513?ïž|+±?‰Ööƒ	O?ˆ`ûõ=¾?‰Ööƒ	O?ᅩH«?ŠZKƒ4r?€íÕ<{x?ŠZKƒ4q?ìHÁƒ,#c?¨˜Æa õD?½¹óæžäñ?¨˜Æa õE?ïÿ˜u?Sc?
ÐFl }n?	â°+'so?
ÐFl €3FGL J0850.0+4855@eNù?ò^W@C£ïÿ×¼À8hìt2À;oÓ £äv?êxÛ¯iœ@Æûþ¿ö@vž_|s¿áœej¬¶¿âå0
ö¿åB™OœËR¿ã8íÉéåÚAGNbllGB6 J0850+4855@?ïúÂåZ\?R)Ÿæ*öG?G¸ôj–"?R)Ÿæ*öS?ﳑ…
?ñVÏÔ:t?ƒž¼º8ü?ñVÏÔ:t?îÓ¥$X?š:,&†F?£ÆÅ­º~[?š:,&†F?ïû¥1È38??	왈F¸?Ak8ß3!¾??	왈F"3FGL J0850.2-1214@mÕ¥€Ãÿ@3‡aÿÏX˜À8#¢á@øÀ;'\Ôm*?öÄxWª‹Ú@C™DµÃ@R‹Ö7"§¿Þ+¹½âŠ_¿âÀûˆLV¿ä¹2X9Io¿èܟEðAGNfsrqPMN J0850-1213?ïÕ¥‹0óö?r@˼eÔà?u-:g†Ž?r@˼eÔá?ïÝ+ò;(:?{/7œ»Íà?qjâkãÈ?{/7œ»Íå?í6®¤Õeû?¦[ÅìF»?¶JŠÙTÐ-?¦[ÅìF»?ïþ¥ÛÙýH?&¢¶Õ©#?%¢B`+ƒ&?&¢¶Õ©#ž3FGL J0850.2+3500@g‹gk*@CBî¤ûÍÀ:—6JÿÀ;÷3I¨Q¿Ñ›>ÎË]@ÁläÚµ™?þ¼òÿçVf¿ë>rH"¿Å¯c)ü˜¿Ï",¹úì¿äÏ$;&OSAGNbllRX J0850.5+3455?ï÷ä‡ôØ?Wv€mº0?P6ðüP*?Wv€mº$?ï]G:"{?'¿Ñ$Ñ—?Œ¨®1waX?'¿Ñ$Ñ—?ï"x%Tš|?"ê0«1ô¾?‹!öªÙa&?"ê0«1ô¾?ï»'<0?y¢@Þ¬<?>[½ðó·?y¢@Þ¬<3FGL J0851.8+5531@d>—?·¥ô@Cx†¿¢AßÀ:2)ösDÀ<¢nTqq¿ý<ÒvYùq@ó!i1Fõ@½3@IFE¿ç«—SKà¿àædçn—¿ßI°¹¬ð ¿ìéìPS](AGNbllSDSS J085135.93+552834.5?ïv—zÀu?œ	‰õ?'-§üK?œ	‰õ?ïÂûö8<'?ˆóÿé•L?~'ãá¿h?ˆóÿé•L?íÁL~')?¦9 Š7po?±õœÞƽ?¦9 Š7pn?ïÿtheŸò?D{÷ ¯?róL¡R?D{÷ l3FGL J0852.6-5756@q5X ÕúÀ!ù€	$ÂÀ8иϿÆTÀ;Vóâ»K›?é¹òïÔ6@·÷¨˜@9ùŸ"®ž¿â3ªÏ¡éI¿æaBq>²¿äòŸ¿Îa¢¿æ*í;¾XAGNbcuPMN J0852-5755?ïú€ªÀÊ?D$ã!éB.?EýTü×Ôö?D$ã!éB1?îô,WB—?¬~äu? ¾M:‹Ö‹?¬~äu?ï.·Pˆý?'ɸŸ?œZ)îàq?'ɸŸ?ï­¡šÇÓB?s…l¨c??"—™N/O?s…l¨c?3FGL J0852.7-4631e@p§Ü_|gZ¿óº_y5À6£Æðù²À9Ú¯ÿ6¬d?߬÷šU×"@",dŒòl?ÿ6í棿ÝßtDJ‡¹¿äjñER¨¿â²à6áé¿Éx/fŸò#OTHERSNRVela Jr?ì¥ò#J"Ò?¼ëÜnnõ?ºÐnå«au?¼ëÜnnõ?é MÒàP?ÏcΪâT1?ɶȴ~¼?ÏcΪâT1?é¤Í'4=Þ?²sõ%mÌ?ÉlËc/‡?²sõ%mÌ?îþUö…ê™?Ÿ>ªZÄa?  —¡Vx?Ÿ>ªZÄ`3FGL J0853.0-3654@p2*Ÿ{Zê@ÑÍÀ<ƅÀ9IÏQâJãÀ;C*3<m¿-|ð(@çúU:n@yÀšºV¿Þ[âòí¸¿Þ´<	œX¿ß…±.Ov¿âe `jAGNbcuNVSS J085310-365820?ï˞Àå—*?{E"r¹ÿ¯?z0Ÿ4j{?{E"r¹ÿ«?ïqs%RÞ?Ÿ1<Éx›‡?'ÑŸ[U¤r?Ÿ1<Éx›‡?ï0O:6?'?maރ?™öx¼,?'?maރ?ïFŽ:pÔû?ˆÕ-x³Ó?—.8±å`±?ˆÕ-x³Ô3FGL J0854.2+4408@fÀ‡D,@D	e4Ù&À:ô°ÿèÀ<Ü»W?ߚÖÌf0È@íÀÓg?ü󚜲ÿ¿ïþ˜˜s÷?ïí–@ž«§¿³'÷þm¿æô·µ8†"AGNbllB3 0850+443?ïÙé¼µ?{£ãÁ‰M?s!öô¦?{£ãÁ‰N?ìúÙU‰ì?ÁDÖ?¸)5S°›š?ÁDÖ?î䖓¸]ï?™9¾¾ŠªÇ?¡¶–Äz!?™9¾¾ŠªÈ?í­GçC3­?¬â>A¤©?²•ÀÅæb'?¬â>A¤©3FGL J0854.8+2006@iÙÔ?u'@Aèä€G¸üÀ7'tvÊbÀ:ÕaèRdQ?óÙq±s*@ÜÉ܂wi@žåE¿|Ø¿Þ¤Sʋ·¿äL
2n¬¿â.V#Åyi¿å
•Þ½ÕAGNBLLOJ 287?ïý1ç˜×?:ÚÚ˜¬?6pÃ9GYõ?:ÚÚ˜¼?ïÇöé.Òé?"§¡ü°	'?|‹h–‹ï?"§¡ü°	&?ïh	)ª¬?Ž/SN¼W?'þÜZʪ•?Ž/SN¼\?ïÿ Äj?V.ô°?û?åžÉ?V.ó#3FGL J0855.2-0718@ma¿ "_ž@7SÎß̃ÒÀ:º$TÀ;ÅÔî~:?èäÄÛfÃ@ Ì@Šà@…#`,e¿áèyÛ°ŒÈ¿çq÷¦a {¿ë&þ¿ïñۙ2/lAGNbcuPKS 0852-07?íÞÂZC?¸—	T×e.?³÷9	í-ß?¸—	T×e.?ÝûIØìŠ?ÑåHj™…W?á[|"‰»?ÑåHj™…W?ìْ¨¯°9?¥‰ç:SM³?¹3jº'~4?¥‰ç:SM³?Êìaâ,?³c‹æõ»?éDç‡y[õ?³c‹æõ»3FGL J0856.5+2057@i¿¥_5½@B?l?Ä;.À9²E¯6¹ÐÀ;!¸·l¿ë;¯P @À7·Qex@|Ì¿`Ó¿çéO?Ù¿ãdÞKy¿âkt}UkA¿Ü-I~AGNbllTXS 0853+211?ïþs!LÇ?#M Tp>?(ÏÝë3‡Ž?#M Tp¡?ï˗²µds?"ØÞ!LW?z4&¥MÆd?"ØÞ!LW
?ïÄIŠú¬p?}k.Ê߸?}Û:'©È5?}k.Êߪ?ïøΓûÈf?KÓðx*Â#?LÅ°ÞfÌ?KÓðx*ÂF3FGL J0856.7-1105@mÔ¾ Ìÿ"@5}c`!¨ÇÀ8Ku€µÀ;ºßd?ð5`ç÷J¥@Á©Æ˜@gUê¿Úfñ£N'¿àúÑ©Á*¿à>'D´Ý9¿äYìý¼%AGNbllPMN J0856-1105?ïýdù{>?5ª5"?4Ø3"& 3?5ª5"E?ï7¨à4×?¡P@ÿƒÍ`?9
ãùe)?¡P@ÿƒÍ`?ïXÃ{Ö&?'˜ÓÒóÚ?"çžð…;K?'˜ÓÒóÜ?êà­8öy?ªú¾µª™?Ä}K''?ªú¾µª™3FGL J0858.1-1951@nÊ?þó†@0‹hß½jYÀ9N^¢LƂÀ;€ûŒ3€?æÙq/‡@Äf1¸3ä@³¢ ~e6¿å¼áÀ­bW¿ã8؊ßÜ8¿ê],¿.\<¿átùg=.'AGNbcuPKS 0855-19?ïùkK§bp?Qcp¾?JRÑbv@<?Qcp¾?ïך¡ÌÙ(?|hfï_í³?t2¯"kã?|hfï_í²?îú¨ÁŸ\[?"µªVâ)ê? Usæ
:??"µªVâ)ê?JT@Òw?t•H.6?€ÕjïËbS?t•H.6	3FGL J0858.1-3130@oô/ ê[S@"p@Õ³PÀ:Z­ã×À;Jaοõ5D°^,@â?j¤
¼?û³˜Þ³ª¿â8[¹íª›¿ãyù»Ã:'¿ÝÌ̀i?¤½Üfj:AGNbcu1RXS J085802.6-313043?ïûPnäŠ?DÅÞA?B¾Do¥ÖU?DÅÞA]?ïڌͶ@`?ˆ‰ßÊÊ%e?r¹™$ßÐL?ˆ‰ßÊÊ%f?ï­A"Y,Ÿ?l̉uZ?"¯šé´Ø;?l̉uZ	?ïÿW«öù_?%7$Ù5:?
 ÓöG?%7$Ù5Q3FGL J0859.1+6219@c%°_®¼A@C?'à°«À:RV	!òÀ<wJº8v¿íÒ=؆G@àc¶Þ£å@u‡_…K¯¿âÛ]ë‡fÖ¿ìąz¶?¿Æ>ôff3¿êÔeè´ÒAGNbll1RXS J085930.5+621737?ïø0¶ö?VÙfÄïéö?O='´'´û?VÙfÄïéü?רּŠýñä?ŠûHMÈם?"Ý@ƒ‡?ŠûHMÈן?ï5Ú#¤9?•†xÆ€?™D»‹nØ?•†xÆ€?ïõ¦(f&?S"ޣ結?T³¯Ï3²W?S"ޣ絑3FGL J0902.4+2050@iÕ³ S\ž@Báj@ºˆÀ9Ñy÷ÜÀ;w˜³ÀŒM?ãjñÎÂxé@~<)Ñàˆ@Б_äA3¿Ô	V'
¿àDÚõ{äõ¿â
C	÷Æ¿áhCÄ×OAGNbllNVSS J090226+205045?ïýÍ«jE?0Óûr®?1'¤¯uÚ´?0Óûr¸?ï±|´zÜ_?‡"®¶§"ã?ƒ ÒáHçÎ?‡"®¶§"ã?ï—#·¾B?…g
š‰V?Š79RoV?…g
š‰U?ïÕåw8?{k\0þ‰ ?Œ
†¢1Ü?{k\0þ‰!3FGL J0903.1+4649@e¢£¿ø¨ô@DÊ:?–îÄÀ:ªÐ"£À;þ>Ëí©¼ÀÈô>«·S@b{üû"@ꀿƒ
;¿å̪*éì ¿ê§B5sn&¿×ÏE%V¯B¿ïú´ù¾¿»AGNfsrqS4 0859+47?ïîAE:ÏJ?nø{ÉwG?a¾ºÅ0·?nø{ÉwG›?ïÅØ;`Å?Œâ=öØJz?}sâOž%?Œâ=öØJz?îÈ«
é'?X6 vÂ?£~…OQgï?X6 vÂ?ïÿõÆþ>ìgNúw|æ>Õærù>ìgNúw}3FGL J0904.3+4240@fSÔà—"ì@Dña_–hÀ9øE~RÀ;åٚ:©I?و]·k;¸@j3óL"W@ο¿É?¿Ý2`Ov
¿ë¬Bn~¿áàʐÀW¿ãÖ–íAGNbcuS4 0900+42?ïøþƒË]?TÁXï1"Ô?LðҋâÐ?TÁXï1"Ô?îjCpÑ]Ù?±Lå1 Zˆ?©[Èòê"?±Lå1 Zˆ?ïÊòÛÈ?•Ä´J¯3G?Ÿf¡¤†þ?•Ä´J¯3H?í{-±RÄ?¨y
M"Ý?·L&'uiì?¨y
M"Ý3FGL J0904.8-5734@qA¬à2ÛÀ! ßÞøHÀ8W,ˆõ¨À;.Ãø贊ÀBjØf@Tꙇ¸@›ÀSu¿æë!{r3œ¿â<>.äÄæ¿ãëË'(Ù¿ÞÿM»8êAGNbcuPKS 0903-57?ïþM·Ý?1#Sk/Û?+$'.—,ï?1#Sk/ä?ïfeäÝ=œ?¦-TTŽ?"3CdXL{?¦-TTŽ?ïj¿lá²Õ?ŒƒãïüM?'¨cÉ¥•?ŒƒãïüI?ïÿôWÞ¢>åôAËôj>×PB»ÒcÌ>åôAËõz3FGL J0904.8-3516@p7߬£b@R ß´+À8¤ÌHBŽñÀ;NÞ̀Pó?çB4E,@Ž )֓@4TçÑá¿ä]ÅÀ¾÷w¿èQKòœÀ¿è	YQnÌU¿ëÉvBÉˈAGNbcuNVSS J090442-351423?ïïO"ò'?]vÐN°?`°lã
ÚS?]vÐN¯?ï¤oºxæ?"ú͇/¥E?†äaýb?"ú͇/¥E?ï)Òoïâú?'þë
""Ï?šÅ² Ë?'þë
""Î?ïx±Y?€çáՊfÏ?éÜßü•?€çáՊfÐ3FGL J0904.9+2739@hÎrà\̊@DE À:W%ô†O:À;å)äÕØ¿øĦf%Ï@
);}"@DßX¿¿èfŸ=ò2¿êqȜçVç¿à4>&}Ô¿æØÿsú3ôAGNfsrqGB6 J0905+2748A?ïý£•°qk?;­=ÓÝ?2ãR|tœ¤?;­=Óö?ï‡p¨1vF?›¥•ö`›2?Ž#Õó¢nª?›¥•ö`›2?ïds¯F"‰?Óẉ:?"qŠ-nÙ?Óẉ:?ïúfŽ«d†?Kýy†ØwÂ?FeÅRmð3?Kýy†Øw¦3FGL J0905.5+1358@jàÓ`Ð$p@AúQßƤ•À9öŸ..À;B̺XV¿Ç½úÏñ@"gtƒ_›?ýknî1÷?Á‹á.Gà¿Ü¼pá6Æ¿Ýĺ]€¿Ôš:YÔBôAGNbllMG1 J090534+1358?ïé†pF™ñ?hæsR+Ñ?fy¹f"?hæsR+Ë?ï½|~Ùæ?‡"‡†ç±Z?€¼ àI†€?‡"‡†ç±\?ïYÓÆøä?ŽÆÞ춌k?"Ň?@ãn?ŽÆÞ춌l?ï˳ÞZD?s\›DwL?z&ôÒÝÏ?s\›DwI3FGL J0906.3-0906@mËýàÖo
@8• ŽÀ9l'^;õzÀ;ƒ0"'¿ÀõTͯR@-Ñ4§@, šTU¿Öø±*"¿âû/–pšG¿ßi²·#¿ß:*šÐbAGNbllPMN J0906-0905?ï÷%È9n?RöZÆ?Q´oá"[?RöZÆ?ïÑT¬È¬?€ï¡'²¦l?wU©›±)ç?€ï¡'²¦m?ïqâré}½?‹E¥:~>¨?'ñ¢ÐHV?‹E¥:~>§?ïÕ͟ò—?iR!3¡?u0q´ç?iR!3£3FGL J0908.4-4916@pä˜à†8¿ñ(Hÿ"_{À8r.ÎI¤À:VZ°O¾"?ä³m»@ÚÍÉwê@"]60¿¿é'íø…Q¿ç׋—£J¿é÷a¿Þõ^®XÛPSRPSRPSR J0908-4913?æ|ùVVÐB?Ë&¨Þü|?Ó
SR_{?Ë&¨Þü{?á¸Ë	½É€?Ó¤rX[–?܎iì"lý?Ó¤rX[–?ã+wöªNž?Á'*€iŸÜ?Ù©«bÆ?Á'*€iŸÜ?êe[¼69w?¸Íel‡OŽ?Æj''"?¸Íel‡OŽ3FGL J0909.0+2310@iŽŸ¾vÉ@Cö?µ!µÀ9š@€MÀ;`¹4i"¿ü
½áÍe@*ÏÝMy?û`àÀt¥¿å¥<Ê¿ä9÷;D"¿ª¹;9UÐÜ¿Ônô'¥AGNbllRX J0908.9+2311?ïÿ§©fçõ?ÏÕ?¦Fnc?ÏՉ?ïÆøâáµ:?ŒD'¡Æ?|ƒŽ%bÿ?ŒD'¡Æ'?ïÑpcÀÊ?M³Q^?wGÎ|Ÿ›r?M³Q^?ïÿ÷C‹91>àöž¥Eö>Ñx鍛û?>àöž¥KÌ3FGL J0909.1+0121@lžj_"ÊÕ@>íÏ ¼£ŠÀ7Ø:ø‰À:Ì;ëh™?üj%
%É@uÔÔÙ
É@AÔÜ:Óæ¿ã'xµ•Åò¿æ–èžÜÆâ¿åFi÷óö¿î5 é¼iAGNfsrqPKS 0906+01?ï1ãùw'?•nRëì?™Ãœ Ñ?•nRëí?ïÂýšäT
?‡"ÓO|9ü?~2Õú™?‡"ÓO|9ý?ì%öD›ò?¦ª/ 1íÿ?¾ÐMß3 h?¦ª/ 1î?ï"=/C"?'ÓÙäH'?›¸Z}€?'ÓÙäH'3FGL J0909.6+0157@l_ 'á@?W°?ÎL)À8û̈Ú.µÀ:îÁðи?ÙÅc@0
¤@wœÄœR@T/ŸªÕ¬¿×ÀÁ`¤Ó¿è¡ ¹*zõ¿ãOÿô¹È0¿ïþÎSNusAGNbllPKS 0907+022?ï'U,?¡.?™‰Ç0¼?‹ª´ð´?™‰Ç0¾?îåFBË~? F×f\l"?¡«›ß£H-? F×f\l"?ëpTð…Y?­ß¿è‰?Â>¬=ꛂ?­ß¿è‹?ì£Kóé¦+?©ãÆU*'Ó?ºå `²Î ?©ãÆU*'Ó3FGL J0909.8-0229@m9pޏ@=ìð{(À8Æ,p¡RËÀ;ƒ†.'ÊJ?øA¡^›@ŽßZn
 @"•úR¿ׯ"[ê¿å9Z£æa¿ãÏý‹RüI¿î'´m–—˜AGNfsrqPKS 0907-023?î+âþ{¢?¬gMb‹pÚ?­AÐGåÜ?¬gMb‹pÛ?éæQr\?ÉѬ
±
?Èfº6Ýþ?ÉѬ
±?æå
õ)ñ?µQVÁ&ßU?Ò5ëଠ?µQVÁ&ßU?åsâCÛç0?¹ÝåC¿>?Õ;xH1 ?¹ÝåC¿>3FGL J0910.5+3329@gã×@Än@E:íàBËWÀ9!þW‰TÀ;T4£u»n¿×,If»4@oÀ£ÉžD?ÿ¿/ •A?ßàÜn€fB¿åwuÂÏÈÖ¿Ý1i¿Øτ!¸6"AGNbllTon 1015?ïþã8—‡?"ùvÐ_¯ù?!Î<v‡¢?"ùvÐ_°K?ï±4w´Xs?o7Žø?ƒ²âéã·?o7Žø?鬒	Ž­?"¹©WÕ«æ?…½œµ?"¹©WÕ«é?ïõ"tá"?Ot×oò–?U»ð<Ø?Ot×oò¦3FGL J0910.7+3858@fö@ÈG,@EÈ?ŸR@À:á6U&£À<]\Òhî?Á8Tú3@Vöï‹Ã?þè`§	Å¿àò
·'$?²'Ÿ¾2…¿áø@{+¿ÌhØÞ VDAGNbllFBQS J091052.0+390202?ïÀ{@z*?…œ¦YÇÿ?Â_Âøêß?…œ¦YÇÿ?ïàÆpĞ?©º+¿ŽÌ=?ŸÃç1çl1?©º+¿ŽÌ>?îŸRÃÛÈí?ŸÃìŽ<?¦
ÓÂCqD?ŸÃìŽ<
?î"lÆgþ½?žž|Íë-?¦¹3™€2?žž|Íë-3FGL J0910.9+2248@i¢Ÿ<pÊ@DƒڐÛÀ9'4èÀ;—;-C/?â=€á^K²@ŠT‰š"@É eϿ׋ͮt2¿ãtÂ6ñ®®¿çuᚌž¿ë_[XÑAGNfsrqTXS 0907+230?îÚTþ/?¢:âøÔ?¢Z¾ðí"?¢:âøÔ?ﯘôk•?~ʊ©°?"?™Âå+?~ʊ©¯?ë¥ær?©ý&b'Òo?ÁhgÞ7ÅÌ?©ý&b'Òp?ïˁÇø†?px¢H,¾	?z?wœ½?px¢H,¾3FGL J0911.8+3351@gÕ¦°)(@Ec—tüÀ:7‹dL°³À;™¤µVŽ'¿Ý/¬	Lž®@
bmÔï°ý@Ììš"ì¿î7á…ä¿«ÈMÙt¿à
_¿O®¿×ÏI_«cAGNbllMG2 J091151+3349?ïùqã|·ó?E
 ƒ(="?J8r
 =t?E
 ƒ(=©?GO¤2?Ÿ%‹r>:ç?Óî,ó'?Ÿ%‹r>:æ?RÎ?†ÍíÆÀi?Œ\þ+}|?†ÍíÆÀm?ïӆÇmJ?q°up¤N?v<œuI[d?q°up¤M3FGL J0912.2+4126@fŠ¿ðEx@E«³ß•ý-À:_›q
.À;ÛßÞèX¿ÍÐU5¼@
:MXÎM@Ч ¿ê™'Îr‹°¿æ	7ÖÓXO¿èÕ5Ú"©?–sáÏwQAGNfsrqB3 0908+416B?ïÿgtf·?l‰îcŒ?s)_:?l‰îcl?ïºCˆˆ&›?7‹1"â?oÝöY;?7‹1"â?ï̧¶ñ?ywnˆ‹i;?yõ¬$ð‡÷?ywnˆ‹iG?ïýÃ_3‰?0écOʔ?1åŽc°?0écOʔ3FGL J0912.2-6452@q£˜¿pÀ&~wÁ½oÀ:
ÑÒÆÀ;­QU])§?Ú±¿ë³@Óá:(@tߥíe¿ädùŸÕE¿êÐKÝN¿Ü|í¼[u¿êÏœ'r^OTHERglcNGC 2808?ïß
#ŠH?t¼ô×~|?pyqn:ÜH?t¼ô×~z?í+ˆwÿðL?¾úFYßYC?¶£¼@}¤?¾úFYßYC?î±Ôa'ž?™å^á0Yj?¤î¹æÖ#?™å^á0Yi?íø67f±?œt~Ç	–?°>ODÊ{?œt~Ç	–3FGL J0912.4+2800@hÐ_ôö@DðãõhÍÀ:sḻôÚÀ;¥Á*[J?êpl÷м@¼™£Õˆ?ø¤¨¡s3?ïýð'
g¿å#º'ê»Ü¿ã!W:é?Übö¨œAGNbll1RXS J091211.9+275955?ïí+öëڙ?p¿‰b¢]Y?bÔ	%fê?p¿‰b¢]U?ï¢þŠÜ—š?•Žäñõ%?‡@]HÚx?•Žäñõ%?íîϙ‡LÉ?¢m:w?°‰ƒ3ř¯?¢m:v?ï'¨ì
?'FvdfR4?‹›ÕÄý?'FvdfR53FGL J0912.6-2757@oß<`Ÿ@+×n Ç‹DÀ9Ì(—ξÀ;—A<á?àÍåù;=@ƒhÄÍ$@"ö`o"¿êI:Û
$¿è–™*ø•í¿âV¬ƒ~¿Ýºfá¾ÿãAGNbcuPMN J0912-2752?ï÷fþ#ϛ?f'+¹QÉ&?Q2¸`Ê4?f'+¹QÉ"?ï}"eü?˜»o¼¯¶?Œ šæ½ø?˜»o¼¯·?ïlÁ"Úׅ?‹Ÿž(?'gÍd¥q?‹Ÿž(
?íÜcÀ9A÷?¢È®àŠh?±áþ5ðJ?¢È®àŠg3FGL J0912.7+1556@j³|€"Þ@C)è°ºHÀ:dÛé*ÑÀ;><{±Q?ÛÐ?фË	@ïK"é!?õœkþÖµ.?䧸ò¿åÍY(¿ä¤ÖFE¶?æ«9åUAGNbllSDSS J091230.61+155528.0?ïòçyî"?c€(cØi§?Z1
â"ùÎ?c€(cØi¤?ïÆê›0.?…LjJ\G?|Š²wçéõ?…LjJ\G?î=@7–Äÿ? 9©k‡*Ê?¬+ü†"°? 9©k‡*É?ïôü#¼Ò?^o‡Ÿ³)Q?V¸†[Í¿?^o‡Ÿ³)A3FGL J0912.9-2104@o3b¯È°@2zeÀN9IÀ9.66òÀ;Uv<?A¿×Í.E|z¿@«%󄜇?ÿä~ð ¿ã°ïÄsŒë¿àõíSļø¿Øõ@gô¿à¨&¿AGNbllMRC 0910-208?ïú£É¤åó?A|n²]ØÜ?EpÙlh3?A|n²]ØÑ?ïÓü³=$?€ŽÇìMÃ8?v±&amK?€ŽÇìMÃ5?ïšÉ+"áb?†ŒyCbY?‰Mµ§a?†ŒyCbY!?ïÙNR}ù?n替™j?sXÖñA!?n替™i3FGL J0915.0+5844@cŸVŸI@D¬à f§ÕÀ:®…à19À<%çbzH›¿íªf@%ßã@ÄÊ7J3@ڝ`˜¿ä%Š9eŽ¿Þ$Žq¿­L¿ë†k‰2e¥¿á錐òAGNbcuSDSS J091608.57+584434.0?ëÆzK|—ˆ?Ç·Ó?ÀæÒ
¡ä?Ç·Ó?ï ùDu°?"ÿ>åˆè?‡Á®â"ú?"ÿ>åˆé?ëô"_ÌZ?´²™ÒÞo?À/wҀΘ?´²™ÒÞo?ïכּ¥nk?]½ÄX?`SDZ'";?]½Ä_3FGL J0915.8+2933@h"žà*w£@Ewa_–hÀ8yœÇ]!À;ãÙq÷¿ÕF¾1­«@!B"ãÒ?þFA,ðú¿ÜÙ{ÞêþÞ¿Ûçª\-2¿Þ{å†#'y¿×+jš8âAGNbllTon 0396?ïéLJӢº?eÉÊÿ£(V?f8x,]F"?eÉÊÿ£(X?ï~™P!?"çÞxTã?‹ú Y«÷ž?"çÞxTã?ïe5&rõ?ŽºÁ3ƒ`?"Y[1¡]ß?ŽºÁ3ƒ`?ï·ÿ…
4š?Ä
†¤É
?'½rÙµ?Ä
†¤É3FGL J0916.3+3857@fø{€©Þ‹@FÁ?À:qGZ1¤¾À;ð¨á59ž?ádû3ßÍÓ@ZáZxq@Ùhy?í[éTlê¿ã¾grJ~¿êÃa›³¿â~¨ÜŽAGNfsrqS4 0913+39?¼àý?"š•ÎH?‰~ßÐÇÁ?"š•ÎI?îsìF‰Ô?±:GëY·?¨ÏÑ;—b·?±:GëY·?ì¨ÓqÎô?°Wàà¼?¿Ê¹dqˆ\?°Wàà¼?ë\ÐÒ·Ë?³ˆavÓeÓ?Œ¼·ù Ô?³ˆavÓeÓ3FGL J0917.3-0344@mfˆ_Js@=äÀ_×,À:d7EçjÞÀ;²ȼœÔ¿ïµbXBiå@mó‹R"?ü7ë¿+N¿é8}RÈO¿×9[B"Dã¿ã–>¢@öÚ?¶ºÚM
AGNbcuNVSS J091714-034315?ï÷äæ¾÷,?QÁ¬žqÍ?P62'§Ð?QÁ¬žqÖ?ïÛ6P®æ§?|<9±¢H??rdרŒ«Ç?|<9±¢H@?ï…r¶7¼{?ˆ>,H€Ç:?Ž£Rrá4?ˆ>,H€Ç6?ïþbÔ¡r"?-zusÞåw?)Òµè×Ɋ?-zusÞåp3FGL J0920.9+4442@eö*?K@Fg€iFëÀ7ƒLŒ ŒÓÀ;6K\äÈ?üÏ͍'ùg@â$Læc@ž–Íar6¿àÎ"Ž[‰$¿å0ðÎ3Õ¿æôc6'§¿êUYyK£öAGNfsrqS4 0917+44?ïã$$‡
?hJªµ¢Â?lÛÛxóô«?hJªµ¢À?ïºH;Ø?Q²»®?mýñ	ú§?Q²»®?쥝SháW?§—ÞúXî¤?ºÓd¸õI?§—ÞúXî¤?ïÿ>¿Ì7"? ›ùèuø?(yxâ? ›ùèvƒ3FGL J0921.0-2258@oŒ¨€QÉ÷@2¥`À:Í~	ZõÀ;ÐNË?.?ðVGšs^G@Òܚu6¹?øÙì€nF¿îØ]Ø´s¿ïÿY<ÛÞ?ïÿd3Rµ&?‹VD"ÍéAGNbcuNVSS J092057-225721?ïöÌK!Ú?a'RÿFí?RgiɼK²?a'RÿFì?ï̈́YÔl?‰eŸ£6ŒÈ?y=Óɱš?‰eŸ£6ŒÈ?îE˃x‡?¡lŋª?¯{£GÈwž?¡lŋª?ïÚ¬‰-{?ÝT7Œý?r©ó;iB}?ÝT7Œý3FGL J0921.8+6215@cúâ~@D'¿ó vÀ8݂ßBñÀ;ÏùrGE9?çþRåÄÚ)@ñÚbâx[@–sßË­¿âxõ7'«Ê¿æÀ¯e2ߦ¿å4eè'%1¿ê
,ZÉGAGNfsrqOK 630?ïü¬:Å?9ÿîðޕ]?:ž)×ÐÀ?9ÿîðޕ?ï"Ù`Î?"#kþ?‹;‰¾§Ì ?"#kþ?ï‹ÉL¦Ûì?‡&%ûU?
¬ÖIò?‡&%ûT?ïœøXvªt?}'׆¹à:?ˆÁéâUcI?}'׆¹à:3FGL J0922.4-0529@m¶<ßï¿@@=èKŸ:ÃJÀ9°)3ÕðbÀ;±m'ª'?¸djÛ£@£ûùá@Y ÿ~û´¿ä&B×7¿×§¨%"¤¿ãÃÍZøZ¿âÏ1,·‡ÛAGNfsrqTXS 0919-052?ïü@¼Z±'?BÌoö¶?=ú*swc?BÌoö¶«?ï¿Em"?'gt+¨?[?€.¤¿wö?'gt+¨?]?郞
Ÿé?"Qëß] <?…Ô|˜˜ú?"Qëß] A?ï"4Ðäċ?{TÂÀê4ü?‹2ËÆÎÝ_?{TÂÀê4ú3FGL J0922.8-3959@p•É 'RT@ѿÀ9ŽaêÖ£À;n©›o\¯¿ð`ëeU@8¶*@žlŸ~"¿ë@†NÒ寿ãÃ¥×?—p¿ëõØùù"8¿]Í­"Å–ÅAGNbcuPKS 0920-39?ïõ*ƒ©Ü»?[s'd?Uªø¬F‰õ?[s'f?ïÏ«·
u?Š µÈ…g?x*1$yEz?Š µÈ…g?ï+Yg$?'ðNi?ŸZ"Ó`?'ðNi?ïþ ×s-?/âx¾4ÛÀ?/ÍòˆÍ2–?/âx¾4ÛÄ3FGL J0923.1+3853@füÜ@W@F´ a3÷À9Ï¥ôïpÀ;Ðbƒ'Öß?×â
ˆçg$@:–n*@,À'wé¿ê¦×>ã!¿æ±ÁäÄíP'•
¶	¿ïþiWVAGNbcuB2 0920+39?ïûuêœ-5?B§h;ÐÊ?B(UK/A?B§h;ÐÊh?í&…4ïU?¸Ëh¿Yr0?¶Ë×VX…W?¸Ëh¿Yr0?ï¨--}5?'¼ †ÒÔÉ?…ô´˜ ²­?'¼ †ÒÔÉ?ês¿¢»ë?³9›2Ý?Æ3•uT?³9›2Ý3FGL J0923.3+4127@f‡Ù!…Æ@F·>À//˜À9cöHòÀ;ȉ¬¼Œ?ßϙ'2@äNô"Í@	3€
&u¿Ü'èJñY¹¿ä–'˜ôX,¿äèZÄFÁ¿ä¬£b¬XÊAGNfsrqB3 0920+416?ïù€Ø+Á@?QÞE§€Š?IüŸPûÕ?QÞE§€ƒ?ïyÛ¦ä¦|?–UÖÖ5?Ä‹#k0f?–UÖÖ5?îäÁä¶O?˜Z«íRÔ|?¡³á´Ÿ{
?˜Z«íRÔ~?ï]§VRÍ?"—šxšS#?"]K5¦j?"—šxšS 3FGL J0924.0+2816@hÛZÀ?ö@F7¿Ý/ñÀ9Æúû´@åÀ;àÂ=&Ò¿êƒ
^Ü7@LÒõÛ¹Ð@^`§"¿å³|ZÍ	¿èÁ­cÈHÑ¿äV&²h¿Ô¿ä™°…™\ˆAGNfsrqB2 0920+28?ïÿ‰Ú54?¨k£›l.?
‰rŸ²Íµ?¨k£›k²?ï¶<çDmí?®52'Š?'pÆ.ä…#?®52'Š?ïÛwp¢ÂŸ?x®0zj´Ç?rDG®ž°T?x®0zj´Å?ïÿ¨V6ƒÌ?gå	ô1?êr_ϸ?gå	ôº3FGL J0924.2+0534@l\
á'6@B'"à4êÀ9ߔãQsÀ;¼Tdc¿¶¸¤®c@,ÁL#å@q·€	z¨¿âwˆ¦Ç¿í3m³À>ý¿½Ç¡Р¿Ø~.ð"ŽSAGNbllRBS 0771?ïÿ{Mć?8Øǎ¿¾?–GG?8Øǎ¿Å?ï̳oM¾?n[HGçæ?y¦HY þä?n[HGçæ?ï̕wåo?y|Å×Ŷ?yµD
uÇø?y|Å×Ŷ?ïó³io‡?SJÌ,€–?Yҙ- ðl?SJÌ,€3FGL J0925.6+5959@cZV`^åi@Eu@ýAÀ:¢,nóÓ¢À;öÓ)ÞÛ?¾']Ç»"@PûSóÈ?úq™ O–@¿ïÿ½Îc?ïù\•W?­¿Ô¯$Æ3¿ÉÝTâãîAGNbllNVSS J092542+595812?ïå¡?j¼¹…eDU?aXLã_?j¼¹…eDW?ïŽ^33v?•Ãª|†J[?Œhs9ó"…?•Ãª|†J\?ïf¢9YK?C:Üè?"+½xÔÖÅ?C:Üè?ﶉukÜB?}·'X36b?']¢¥ïÐ?}·'X36a3FGL J0925.7+3129@hO8`™Ë@F«×à&EåÀ:å? §?uÀ<"6;%oü¿ÄXI÷RÕ@9.oÜ?ÿõ÷áMR¿ßù¥»ïb'¿ç>¥Ã¯¨á¿ºø
é˜é¿æÍXðýAGNbllB2 0922+31B?ïó*€lË?jgTµí"E?Yûªÿ&md?jgTµí"@?ï¢Æve?'³.ÇÙ5?‡N`;âf?'³.ÇÙ4?×fą?£a•TœûÝ?¤¥b‰"·©?£a•TœûÝ?ïäè]p'ï?ipn/ü?k¢ØC?ipn/þ3FGL J0926.3+5409@dM…@FA-@F	Øà†8À:°ÄŸá§À<'ªoª²Ç¿Ü¿¡26«Z@À§8¾o@£¿bV¿Ö[A?÷x¿åuœ#âˆK¿ß2̜ț¿ä÷)攅DAGNbllNVSS J092638+541126?ïørq­»"?_â˜ì›¿?N69Iò»?_â˜ì›¾?ï«ä(O¶«?Î|'Û_?…õìUd?Î|'Û_?îãžÉÍ?žƒð–âÛ?¡Æsn">?žƒð–âÙ?ïí¨×"Z?]!d~-ð?bW(~l¤Ž?]!d~-è3FGL J0927.9-2037@ovýç!@5kjК¸À9 ~¶¿DNÀ;»Ý:ZM?ݗ¿.©‹ª@çk›¦ÿ@ìßfØQ¿Ý@º–z'¿çVá®ä¸¿æþš­ÉZ¿æ¿þ½à ¿AGNfsrqPKS 0925-203?ïþ]Ñ
¸¹?*ÌíQ/Ä?*"ï$tƒÀ?*ÌíQ/Þ?ïÙVœ£&?|R‰ö?sT±®1m,?|R‰ö?ï'ÉŠ?"Ó²'x®?¦ß_.Æ?"Ó²'x¯?ïì UÌ[?Y1S|Ajì?cߪ3í¦—?Y1S|AjÚ3FGL J0928.5+4048@f¤4?¢­?@G5Ôÿ¡5oÀ:¦xmÏç4À;ø˜‡Jâ|¿¬»t3Ž<@
y$nŸDÿ?ýz¹>ÐuN?æèæ˜ðI¿Ìú\ßÌPH¿á+9/²±T¿ÄÔ+j*ÚäAGNbll1RXS J092837.8+404858?ïâê/»T?s<1Ö ?mÐD«äâ?s<1Ö#?ï£LòäK?":´ÂÌGÜ?‡,ÃFí;¾?":´ÂÌGÜ?îÞk¾,°'?˜ŸBb'Â?¢D4÷Ô?˜ŸBb'Â?ïÎlÃ_&?r4{R²\??xÉðPm?r4{R²\?3FGL J0928.7+7300@akO¿ÆT
@Bwa_–hÀ:z²YƒÿÔÀ<
Մ+sK?ä\PZáM@
¨œÕä"ª@T¼ù›¿îeó%•Õ"¿ÚR#îò''¿ã'Å&W$¿éOÆD{
AGNbcuGB6 J0929+7304?ìu"m¬?Â]NNa
°?¼Sß¼' ?Â]NNa
°?퐂émƒ?¹¿í*ج?³{贓çG?¹¿í*ج?ì@¤Jòþ?®€n±Rä?½úßE¨h?®€n±Rä?æN›tGM??»æI6€˜¶?ÓbÉqe'?»æI6€˜¶3FGL J0928.9-3530@ppŸS @&xwàâ-‡À9Yp×ÙpIÀ;ˆÛýÂ8?¬í9ŒÙ@
Ööz°@>5_³Cå¿ê)ýêÑðx¿æB]ÌJ,/¿àF–½Š¿éÎÁb‹eAGNbcuNVSS J092849-352947?ïŸî=¤òË?ŽÐ4%rž?ˆp–ÃLñ?ŽÐ4%rž?ì¹se¨"?»ܑ[‰f?º4dÒ¿ãÛ?»ܑ[‰f?íc€÷G?¦'ã5pJ?·TãøEÇÃ?¦'ã5pI?뎥í@E²?­×º\)?ÁÅhJþé>?­×º\*3FGL J0929.4+5013@dõߨq¤@F¹!¬ˆŠÀ9.$I‹dMÀ;7p¯•"?¿káÝL™-@ñxŠ|E@Pàc, ¿ãI&¢ßœ¿ä㹺e/ô¿ãþ 2K<û¿Í½dqfAGNbllGB6 J0929+5013?ïÿK_"–«?ç"K©}?"­*ŽQ?ç"K©}3?ï¥Ã&Ó?í˜'å‰÷?†º6[Ë)?í˜'å‰ø?ïÕ. ×Ä?vF'½y•Ã?u@h¯"[?vF'½y•È?ïã"·ù½?dƈŸÎ
í?lléHD3?dƈŸÎ
ô3FGL J0930.0+4951@e§€w‰¤@FÐ<aNÏÀ:h÷´×ãÀ; õ§·iŽ?çê¾±kž@ðÜ¡›?÷&€®ç	¿ÔâªÂêSy?ï…Þ7¿å²6ĕÏ=?Ý\–æ®A¿AGNbll1ES 0927+500?íÅì€E?²E/û›Ê?±×П#ýÙ?²E/û›Ê?ïiò-ç@? è,¥±†›?'ÁºCüK? è,¥±†š?ë\ÉÔ²Ê?±¡«ík?Œح7ô×?±¡«ík?î'$Î(³×?¦kOqCÅl?¦í³t†?¦kOqCÅk3FGL J0930.2+8612@_'‡aˆ±@=ƒ¬ßÇ{TÀ8õ̏+\À;¥÷´#ì?äCÄeþ•$@,1â%O@xF€B²¿ÙúA©\t¿âœ‹ó1e¿å"Lu¿á\b'áÚAGNbllS5 0916+864?ïùÉÓæ-?I¤Ï˜îu;?HسägID?I¤Ï˜îu;?ï†Y›¯vÇ?—/:¬¿?Ži™"Mù?—/:¬¿?î·o접?œ@S(¥´
?¤Ž¹5öí?œ@S(¥´
?î¹¹¹:j8?–xgŠô?¤ddlY\˜?–xgŠõ3FGL J0930.9-1904@o^à?pX@6÷Û ¥&–À:‡âÀT†À;ȋfÐïq?ñuõjzÈ@
>ä'åp2?ý—sŸ4
N?ï‡HvÞ¦?ïj#hÿŒ¬¿ÙÞÏuÀîÀ¿é"KaiýPSRPSRPSR J0931-1902?î¯W«6d?¦WÄZ¥‡?¥J…L™Õ?¦WÄZ¥ˆ?ãZÇ؂Ë?ÔäbNô?ÙJqþNúk?ÔäbNô?çï»|c?¸Åƒ*±Ôn?Ñò ‰9Ï?¸Åƒ*±Ôn?äŽV‹Zm"?ƒ4(_p?ÖãRéK%»?ƒ4(_p3FGL J0934.1+3933@fÝ]¿Î·‰@GÅ)ßÍZ'À:&æQÙ¨À;õ¯}0­G?ê·ûקFU@Žµ‹è@8RÝk¿Ý¥ø³ÁŸ-¿á¢¹䏿ãhśwŒ¡¿ìÿÊKÏGAGNbllGB6 J0934+3926?Еµœo«?Ê͸ˆµˆ÷?çµ%{±È+?Ê͸ˆµˆ÷?ãz"‡'~9?ÌVóI ±?Ù
öðۍ?ÌVóI ±?äÉòʈ Ó?¹RÖ·y+?Öljî¾Y?¹RÖ·y+?ݽnbR?·ø§+@¾ ?á!HüN¹W?·ø§+@¾ 3FGL J0939.2-1732@oe'@š$@9v·¿õMõÀ9Ÿlr"À;§þ#†íÅ?ëÉï"Å@ß@V‡7Â9 @(Nß·
C¿àÎ1ÏX¿ãmt‡¼Lw¿áöE"㟿íËaè¨KAGNbcuTXS 0936-173?ïløÝ'Õ?wà,߈S?'`ä[_?wà,߈S?ïyÞï'h'?"ÀX梀×?Ä"
²û?"ÀX梀×?êŒøsÔy;?°Ã»éÈm?ÅÌ0®?°Ã»éÈm?î*Ýrhœ‡?˜ƒw·¥B?­R(Ùv7¢?˜ƒw·¥B3FGL J0939.9-2831@p;vm
J@1Ý!ŸŒø¡À9s£Ô…þ²À;¥7†
¢¿¼gù訏E@…®	Ïã@Åt®¶â¿è_ä°Ëö¿ãe€ûñ†¿äÞn´ò¿ïÿ¤vЎAGNbcuTXS 0937-282?ïì'~Óf?l:`Ñ?cm~,™Ä?l:`Û?ï̵6ü=Æ?ƒáLÇÖÞ?y¥dáæ?ƒáLÇÖÞ?îã'õ$v?¡2͌­Œ?¯Æà­¸­?¡2͌­Œ?ïêÆ?_Q(LÁ,Ù?eð9áèðÏ?_Q(LÁ,à3FGL J0940.7-6102@qGÿÞrÀW MRnÀ9ƒúNw\À;]¯"­¡Ž?ïÄ*×]ä@~ëÑL@^d¿9a¿Ód5Ë$<\¿ãÔ/5]ì¿ê"'ƒöo¿êb-à@¥•AGNbcuMRC 0939-608?¼¾êÞ£?º,Þ¡&¤Ÿ?ìh"¤?˛?º,Þ¡&¤Ÿ?Ùk$JA:+?Ó¹‹ÄP°w?ãJmÚßbê?Ó¹‹ÄP°w?ØKL»¶ÑT?»õm܇dX?ãÚY¢$—V?»õm܇dX?Øjؓp
?´±¯^cwù?ãʓ¶Gòx?´±¯^cwù3FGL J0940.9-1337@okÿÚ@@<g®¿›‹âÀ9«Væ—À;±gž?ÙыÇ㝸@V¹"
ä`@EÜѹ¿áÙú£°Úå¿åû¬'œ¿è'º+×Á•¿àf>"z~KAGNfsrqTXS 0938-133?ïþ™…%gÖ?*Hc*§4?&g­©'§?*Hc*§4Œ?ïыè?€çê•ÍìX?w:@rrw?€çê•ÍìW?ï[JÆßôä?	N';Ô¶?"–§$cv?	N';Ô¯?ïù³2¥Íw?CôøÕu™2?I35hʳ?CôøÕu™'3FGL J0941.6+2727@i$(?NÊh@H
÷Ÿß-øÀ:!>ºOò‡À;øgÕÒ/¿ëŠÝœ±Y²@
í1™*^@õíHû¿æzv×ÞßÛ¿æÆ(»,‰¿å'¬í€Ã׿çÔ`hå5"AGNfsrqMG2 J094148+2728?ï÷¯YŒÒÜ?U÷FÏ°?P¡LæZGä?U÷Fϲ?ïC2^ƒ? ;Áßn«Ã?—™¿ýt/‹? ;Áßn«Ã?ï;_53Q?'¯I(ÒÃ?ø"Y•Ø?'¯I(ÒÁ?ï˯MݑÊ?xu`jÎÃÂ?z(Y7¤?xu`jÎÃÄ3FGL J0942.1-0756@nnY!…Æ@@(àaÕÀ:D"ÐÜýÀ;×Ê0:Zo?î¢Ðƒ6@ʂٹš@@‡}?pÙ1?ïþª'[c©¿Ø9î'N¿äÍExZ.˿䪀;ú'AGNbllPMN J0942-0800?ïû5Zÿ¶·?P«+X«??C*"%#v?P«+X«O?ïÃùÎðÉo?"SƈÅc?~‡›HE?"SƈÅc?íýÉ%ÌŽ?£øœë(?°¶ÑŸC–?£øœë)?ïfÅš?ˆÓäf?"']=G¬²?ˆÓäf3FGL J0945.9+5756@c"`RP/@F¶¬@eJÝÀ9§#Pg ¡À;þEE"n¿ã3ÿ‹æÔ@–K Kz@£	ÛØ¿å_Ð˒˜§¿á·ڌÿ俋8áP›¿ç>eðŽŒºAGNbllGB6 J0945+5757?ïë¸cT?gD'c±½?dGœùú­Z?gD'c±½?ïh7Ý¿9?—Ít³A?'ùHxô?—Ít³B?ïLìö¨¢µ?'ŽsSzéè?–ba*ë©Y?'ŽsSzéè?ïÒ܈ò#?r‰øüÎy?v'»†ònÝ?r‰øüÎw3FGL J0946.2+0103@mlÀ
¡©@CHEßÞ!‰À:•Rh' YÀ;¹Ã›Ë£?ã¤aöÑ>@ëréV›B?ûÏ¡‰Å?ïù«±~Æ¿ïþ±²{N?ïñ´Ï;MD?Ä ¾seàAGNbllRXS J094620.5+010459?ïü§ˆ5y4?E2¹þ'L?:þT6mG?E2¹þ'U?ï¼ÊU%á?ÐÀ¿Uk~?€Íj¼v‡Ä?ÐÀ¿Uk}?ï7«Wسü?Î-W?™
•逍?Î-W‡?ïû£lÝÀ?RúŸJ—?ArLˆÿþß?RúŸJ¡3FGL J0946.5+1017@lïàÎ'@Eµ'ÿùJÀ8­@)»»-À;€¿®Y?ó|
‡ÃXZ@	‡±d¼m@©Ç`&[^¿â¸Œ4<"¿çÑëë1M¿è£:µ¼¦¿ç¥ÞvdÙAGNfsrqTXS 0943+105?ïø~05ˆé?Qe8Æ?N?)ÜZÇ?Qe8´?ïxs"êY?¤#E/å˜?ðñ'´«?¤#E/å—?ïMo(&yÉ?'Öᛲo?–Rû0ÆÇ?'Öᛲq?ìF؜uUÃ?«&(ûÆäy?½É;UQç?«&(ûÆäy3FGL J0947.1-2542@p.W /µÐ@5¯ãˆÀ9sHÌølÀ;ø˜,²?Ù¯ËàÏ»@$ko9Ê?ÿ30ßEö.¿Óø«oQi¿ß6N.í%¿ÝV=Fåö¿à겆$œÂAGNbcu1RXS J094709.2-254056?ï»!cš?"º	å"0ç?7§>Ù{^?"º	å"0æ?ïhÄRx?'
jÂ[<?‹åÎü+b'?'
jÂ[;?ï$Óó¯(³?"A2"º,?›eŠéÈ?"A2"º*?îJ
8$<g?"*®´y'A?«_,}¼9?"*®´y'B3FGL J0948.6+4041@fžP >cé@I+ŸÀûÀ9é ªšrÝÀ;ü	Iú¿ü¬iøÂ@ʚ‡«/™@Yÿ¿"S¿çþ€!‰£¾¿çVŒ@낚¿æINa7…¿ïÿñ([AGNfsrq4C +40.24?ïþy¶\?0Y|ËB-?(dš?Ð?0Y|ËB-?ï 	Ia?'š[ØØô?‡à=­¹§Î?'š[ØØô?ï›2VF"?ˆæúQe;?‰3jnZü?ˆæúQe;?ïýþ\p˜m?4º¡lhù+?0
{<"Â?4º¡lhù+3FGL J0948.8+0021@m'Þß)@CXßÿ¯x(À7»¯ºmÀ;Y	Ó¾X–@Ü^žà@V©¡#¦£@é‹+홡¿ãøN§;¿é/2°ßäà¿ê"9Æ^•¿ïÿ
1ŸgíAGNNLSY1PMN J0948+0022?ïð$ªžK…?b	`7@k?_¶ªÃhóÓ?b	`7@k?ï&…)Ìõ?§ö«É"I?›=oZÆam?§ö«É"I€?ìgþ%?¨¤ˆ Êùj?¿ôÇӀ?¨¤ˆ Êùj?ì‰]³˜Â?³9‰^æ}?»µc?¹ð?³9‰^æ}3FGL J0950.1+4554@e›ú€Ïž8@HÜRÿ" À9ù8¶Ç¨À;Õ
¥uoï?Û´þ,žÍ@‰}dBö?ÿ3˜Ì•¿êøÖçU‡¿ÖT©dÊD¿áf¡³¯õ¿Ï'·ïdAGNbllRX J0950.2+4553?ïëí+ä/i?iœ]EœóÞ?dÔЗu?iœ]Eœóâ?î^Þ×Íõ?¶ÞÁîê?ªƒ.Щ?¶ÞÁîê?ï%•–³¶?"n9X
Ys?›MM)‰>¥?"n9X
Ys?íÞ±NÅ ?¥"'ڔ?±
uÙ×?¥"'ڔ3FGL J0953.0-0839@nř'ÿ@@óàVÀ8H.Z†^SÀ:ÙFóÚWÐ?ñ|Çô ÑF@Úú7äž?üâÝø]Ê¿ÊQʑÍâ¿Õ»ÙÂK¿ÞŽcMµÉ¿ÖtËí¿ÈAGNbllPMN J0953-0840?ïü{&oký?BvªlsìV?<&̄ ¨?Bvªlsìl?ï·Y|"?‰)Óßԝ´?') Ï[9m?‰)Óßԝ·?îÈO/ü?œ~ô3RÂg?£{
 >Ó?œ~ô3RÂg?ïxwÃ?‰V"û
ìG?œÜþqÄ?‰V"û
ìG3FGL J0953.1-7657c@rV@ €À1‡@zC"À9ï›Á''À;ü#Òm ¿à͙—Úìd@ÛXè#•[?þ—‡€½Tµ?î"NX&C¿ÊüýRaÞ¿ØaiTµík¿â¯š
hõÉAGNbcu1RXS J095306.1-765755 ?ïïnG†Õ#?aل줯F?`'¸y*Ûá?aل줯B?ï¢,ݖo?"Ñø!'Ð?‡tÿHšcÉ?"Ñø!'Ñ?ïf\.×!?‰"j•~­5?"4|º%½?‰"j•~­2?ï͉bÓy¿?tCŽ3¶ì?y;N–C  ?tCŽ3¶ð3FGL J0954.2+4913@dôªà~Zy@HÉö`D
vÀ:©î,˜å?À;Ë¢1Ð?äL´Ø©Í@°†'¡Ú†?õM9§š¹?îwÂ%Ì:¿ã¤ähŸÑ—¿ïÂ0œÞ{)?ﰋ֍jâAGNbll1ES 0950+495?L@Æ?—&¼OÍl4?‹ìïúµ?—&¼OÍl4?ï/ÔH*?³fóÞԏ?š|VïÚæ?³fóÞԏ?ê€Ëm9›[?³L€'"ì?ÅüÒK'"?³L€'"ì?ïTøºŒ?¡ì¾žQ	?•|è®}¸?¡ì¾žQ	3FGL J0955.4+6940@a®+ÀãŠ~@DE…`&±EÀ9A¢e6À;Ï"כ\è?Ñ9Ô
x@
xjRWù@®#ÿ¹‰#¿ßßëÄ¿ÞTžç·4¿çÑ,ÎDœ¿ÛÄę!¥OTHERsbgM 82?ëû´¶ŸÂ?Àð¹·À¶?À/%€÷?Àð¹·Àµ?éx Ðé"î?Ï<
	vð?Ê|¼Y¬N?Ï<
	vð?éØ1<ëV»?¶1´¥‰#?ȟ;R¥?¶1´¥‰#?åQɅ)À[?íçæÄI¾?Õ\lõ¬J?íçæÄI¾3FGL J0955.6-6148@q»-ÿ'+¿ÀÈÙà0¬ÆÀ9…¦ a4À;dM\‰?êÄG©³@
}~
@›_¿®+L¿å÷ó4Ѫ¿â·K:Þ¿ÛY6ÿ⺿îÏ
L½¦rPSRpsrPSR J0955-61?Ñ¤©‰)'?ÈþnnþÃ_?çy­«;k7?ÈþnnþÃ_?Ð6aY§?ÐÒ2¦âbÄ?çäÏ9S,z?ÐÒ2¦âbÄ?âéÅÀgº?¹o
jÿË?ÛÎ,t0‹?¹o
jÿË?ÞˏÅà°Ï?»·Cê¨í¾?àš8§™?»·Cê¨í¿3FGL J0956.6+2515@i¯?p]@Iwù jn3À9!Áû¸r£À;²#ÃS§G?ðÐój›TZ@ÒPw¹Ë@|G '¨;¿ãGXÕ6Ü>¿äãëSdoÛ¿è_EüŸ´w¿ïÿ˜µÁ²AGNfsrqOK 290@?ïì)ŽÈw·?h6þãC—À?cÖq7ˆJ=?h6þãC—¿?ï«MFR?¨ÁãM?œJ–]5Ò?¨ÁãM?íf>ù2­"?¤õ@Eªš?´Î6j"S?¤õ@Eª›?îŠì%{°?žz¨O{‡?¯çQ=¨Dÿ?žz¨O{‡3FGL J0956.7-6441@qك @ÀÀ'{ 4hgÀ9´Ïú~¶¿À;}hq¡›¿Ó>ehIÀ@wZ!‰'@Ià [R¿å•‹g>§¿é‹åô¿å	=Éí¨¿Ó=X™&àAGNbcuAT20G J095612-643928?ïôK#M?_fo%'?WiÓ¹Ëbk?_fo%?ï]{ö;†—?¢ Ã×ðqé?"P8-5?¢ Ã×ðqé?ïUPE@¨?Ž	ŒlÃY?•U÷Wýªü?Ž	ŒlÃ^?ïß3;	$?gXé›Û;
?pfb{mþ3?gXé›Û;3FGL J0957.4+4728@eA¿p@IIí )k3À:¨(÷À<ÿ™¨³?åðQòċ¾@"y$én@[œ@gú¿Ùftlþ¿éÅÿýËÑ¿ïj'"?ÐÅ@CŠµAGNfsrqOK 492?ïñ×üJw?wþRæÇ›?\Pk,?wþRæÇœ?ïŽÝ©Èš2?–A3€çms?ŒH•Ùs‡?–A3€çms?íhä‡~?§7w8ú?´¸ÛÇÌ	?§7w8ù?ïOŽ›òr?™öåñåªü?–,½£?™öåñåªû3FGL J0957.5-1351@os Æ´…@?.²˜¬4À9_ÄM¢JBÀ;ªFX©åA?öfàý0lÚ@wŸäŒ\@)=³ê¨«¿ás؉ÚP¿æY<Ž&¿ë8ÙP;y¿ïÿ"û&ýEAGNfsrqPMN J0957-1350?ïô‡ëùd?\kÙ'5ÿ?Vð)Ø
5'?\kÙ'6?ï{Z÷NÉ?—ºßkî?"¿!'?—ºßkî?íszrž
­?£öE?´d,kª?£öE?íâþ»­ƒ?¢Jª1	0?°è
""çg?¢Jª1	03FGL J0957.6+5523@cÒó@ÔÜf@GöãàÈñÀ7nû`^À: u'ÊI?øÂjž.@
ûãL@€?ýÌðW@"¿ÙNKÏié¿àšÈ0ŽpÏ¿àÕ£Ñçúâ¿âd»rv-óAGNfsrq4C +55.17?Ð|§Ù]u.?ƅÅw¢Åç?çÁ¬QEi?ƅÅw¢Åç?"¢½‡óþ?´h®l nÓ?ïbëÀ_?´h®l nÓ?âÐV¤îN?µÜaýfG»?Ú_ÍR¶#d?µÜaýfG»?ŽõLn"Â?€\t(È/'?ï"*ÎEÃv?€\t(È/'3FGL J0958.3-0318@nD¸€®@C.^è¬À:uÓ|ê6jÀ;—ÛBö?ç±Ä‹_Å
@
wã'_c?ø=ÖÀ¯?¿éśžæ¿´Á¨Æ!%Ù?Õ<OÞÜç?º¹U2AGNbll1RXS J095806.4-031729?ïçê8µ?lS˜pc?hûäÇKÁ?lS˜pd?ï³{"Ò³?"®"õ)ý?ƒ!8šËSŽ?"®"õ)û?ï4kÌÔ^Û?EbÙo­?™r†et$€?EbÙo®?ïÞúah?sA jèk¾?p'ÏKýÀ¯?sA jèk½3FGL J0958.4-6752@qû™€o&)À$Š>ž¡@WÀ9ûͅYqÀ; ô‰u?Й¼(ÃK@
áJòA¦i@§ø`ygu¿ëK"ÞK¥E¿à`–!ƒÍ¿ØP¿ˆõ?¿ãf"Ú ¨ŠAGNbcu1RXS J095812.8-675241?ïëK£¯ÇN?c¿ý°hc?d´\P8°o?c¿ý°hc?î3²m@?³äƒ«r?¬Î´Ù+öK?³äƒ«r?ïcXûP?ŽÁaÜ%Ê£?""þ •ì'?ŽÁaÜ%Ê£?îéªߞz?Ž5~§Øš>?¡e_'T?Ž5~§Øš?3FGL J0958.6+6534@b82€ñ,(@E&Ÿ¦ùÔÀ8¾­µ°P•À;ÁUÊ6ðW¿øv†PÀb@ÃÖDDÓo@
@?‹0J¿ã•Ó€ná¿åÒÙõ‡à¿ä-Í÷!é¿æ®ƒZµO¥AGNbllS4 0954+65?ïÿ°›ØðÚ?(3AÕô?Ù	ÃÉ/3?(3AՈ?ïɟn~ók?Šn"£<¹ß?{0HÀ†J?Šn"£<¹à?ïáß'Š?rXRopú?nî Øv=?rXRopò?ïÿôáv>åšåÅ&…>Ö=ûÊ¿>åšåÅ&€ë3FGL J0958.6-2447@pDêŽ:Á@7pæàtI~À:
ZÜÅhTÀ;Âá½Ùà?·3Q7Ágˆ@XÓÞå@ðp¿…¼m¿á\ï»Ü¿åºH싌™¿æ\wÜtNu¿ÔnRÍF3AGNbcuTXS 0956-244?ïÍ#;òé ?'JTs:;I?ynb‹p(?'JTs:;J?ï¥éy_Ïá?']Þí‡S‹?†…¡¨?']Þí‡SŠ?îçN…(bX?œ`¬(s?¡‹­yÚ{?œ`¬(u?ïLUT?Œš»>Òæ ?–uU."?Œš»>Òæ¡3FGL J0959.7+2124@jtþKZ@IQ4 ½À:[®a§ºÅÀ;äEÞ0¢_¿þ‡†AM'P@Þä‡(¨Á@) CVí?Õ®ï1%¼Ó¿ß"ç†óŠã¿ë>ãp?›+á
ÈAGNbllRX J0959.4+2123?^è­y?¬Ë:id|?¤u(€?¬Ë:id{?ï±Â?Ù?ÏµT"¶£?ƒp:	?ÏµT"¶¤?ë÷ÝÊñj9?³•_!€óm?À ˆÔ:W?³•_!€óo?ïÿÒ=è`n?úò7 ©œ>öáÏÉá¦?úò7 ©Ý3FGL J1001.0+2913@hî^ß)@JK8_ÂÞ7À9'Ö!à$˜À;ÁCÂÍoŠ¿ô‡XC¸çh@ï1Æ̂¥@A›Ÿ®0ª¿á;™Užd¿æ›Siñ¿áhòüGŸã¿Ó—Ãl7AGNbllGB6 J1001+2911?ïÿä笻>è-MRɍË>ëSDçÂc>è-MRɊ3?ïĨ›$×Ñ?‰Å瀑÷u?}«²m"Š?‰Å瀑÷s?ïàôM'¦1?w$»:G~¸?o²}Yз?w$»:G~¯?ïÿüwó&>ÄP¡E>¿ô@fÑÉd>ÄP¡C›3FGL J1002.3+2220@jPå`A‰7@I¿f€g™lÀ:d~¡ÆÀ;à\d"ä׿ǃ'Ù6Ã@ëþ<[{@x¬ßœˆ6¿Ý]ޞl£S¿ê8Šò¿Õ2–È%j•¿èB`é"]AGNbll1RXS J100235.8+221609?ïüP)˜`Í?H"qHué?=~³<ùžH?H"qHuð?íÕ9´;ü'?¸@•6çJ?±V2^ Ñ?¸@•6çJ?î9òÔv?¤â.ªÞ?®Ì`Ò¾¨ƒ?¤â.ªÞ?îVg .R»?£PrÇØ2E?ª™ýÔ<?£PrÇØ2E3FGL J1003.6+2608@i"&?šIÃ@JV<ã.À:nˆö´&äÀ;ãØ$ãý¿áYZŽ/ÇÞ@
ÃNÿl‡=@UÎ 3ý¿äÜ4~]z¿èñ*,××ö¿Ò'i!à-¿êŒ²$ÒÏAGNbcuPKS 1000+26?ïö^¨Yg&?[y' Ïùv?SB¯M1±?[y' Ïù†?ï¬nµ!ë?¥vÝ+üZ?œªr)[±?¥vÝ+üZ?îoì•]?¢±aþA?©6ª'îi?¢±aþ@?ï¼Ãðü£í?]¨†˜\c?€ÏÀ×%?]¨†˜\`3FGL J1005.0-4959@qYBà°«@
Ý¿ä1À9 –6—À;W¢Õ'}ô¿í¾¾Ë='Â@
çEgée@78¿å׿é殚T!¿èrWý(E€¿ç.ϧ%Pû¿ä"0™[ AGNbcuPMN J1006-5018	?ïæɼwCª?pêf¢·p±?i6Cˆ¼T˜?pêf¢·p®?ï‰5•/ýÙ?¤ê÷JZŒi?²š´‰ƒ?¤ê÷JZŒi?î­a¾_Ôì?—G'ìX»†?¥)ä±;?—G'ìX»ƒ?ïåaàÚd`?eú7™TT?jž%›Ÿ?eú7™TW3FGL J1006.7+3453@g€Àð¸@K6îÍ©À:¾ž\vù\À;êň4íH¿×ך3{
@@
cJØkf€?ú|R@¿Ê¿ïÿ
ç\›?ïÍ"Ê5¿ÔÄ@ٱ뿹ܦ/eY‡AGNbllEXO 1004.0+3509?ïýÈê´1?2Ź—¶S¨?1¸¯š^€Ë?2Ź—¶S—?ï{áôyKk?š+ ×iÎT?ƒÁp֒¯?š+ ×iÎT?ì?…ÚÕ 7µ?ŒUøûÄþ?…ÚÕ 7»?ﻈÓFƐ?ùcb]˜?Ë.N[§?ùcb]š3FGL J1006.7-2159@p<۟˜·@:ȖÀ¡E`À8¹æè¹À;ŒÕÓËò?Åò´âd'Œ@.ÁКaÁ@z›@7Ӂ¿âJ°7S¿çæ `U¿è%=ÍÒŸ¿×Æ*g˜Ñ¯AGNfsrqPKS 1004-217?ïûÜíì›Ý?D5P
[?@ŒHMŠf?D5P
Zþ?ïÓcñÈ%ª?€ñ¬
ö2Ô?vNí*Þ?€ñ¬
ö2Ô?Âe?ƒ"Ùns̅?‡˜zf»É?ƒ"Ùns̅?ïޗ™€ô€?g鸖äðk?p´3?…Àa?g鸖äðk3FGL J1007.4-3334@p¾%`A‰7@1é¬ "ÚÆÀ:Ž(LOdÀ;¥¹¯¹–?ñÃv¤÷ñ"@·T?@N[ÿ…0׿ßúú¾]Úb¿èÕìÅTw¿èq…­Ғ¿ïÿ8Ýl,NAGNfsrqPKS 1005-333?çbm¤Á?ÊVug"!?Ñ;%Ò¶€?ÊVug"!?ãÓçÝÕy?Н©R]?ØX1ÆDU?Н©R]?âÑkp]?¸¬*§`?Ú])ßÃD?¸¬*§`?Èçø—¼ù6?¯å>dr³?éÆÚÁ³?¯å>dr³3FGL J1007.8+0026@n?@OÂ@EFv¹ÃÀ:BôˆÓx¸À;Î))Äõh?×Íí"äg@²A±%@¶'¿t?ïýÙý¡¿å"­·]Ï¿¿×®O½Ç:+¿ç`n©š²bAGNbcuPKS 1005+007?ïü=iK-Ö?@ÆDĎ?>µ¦'Xì?@ÆDĎ?ìIŒµ¿²?¿×£5ÓV?½³ŸÊRz?¿×£5ÓV?ï>•à·è?<&Ií)?˜-Cé	?<&Ií*?êmj¶Í‡Ô?³}ô†mû3?ÆJU$Éà®?³}ô†mû33FGL J1007.9+0621@m00ÿì·@Fÿì@/šøÀ8õ¬Á"ŠfÀ;}X¶zzð?ï½ÅÀ6@Aé;îB¾@@<`ƒxp¿ÚIÿ6Ô¿å9=–ìô"¿åÈ,Ì礿¿ág"j´AGNbllMG1 J100800+0621?ïë¬Á³?n
b#ÝA?dS>ÿâL¡?n
b#Ý<?îeQôê¼%?¯ðp9ÑÌ?©ªà±T=©?¯ðp9ÑÍ?îS´˜Ý]?3ÎŽ	n?ªÏ¶r*3?3ÎŽ	l?éb½1üÝ?²U¨j?Êu8‹?²U¨j3FGL J1008.9-2910@p"íà
q@5cÿƒÙ>À:.'Gl¦À;ÄÁE°
y¿×ÑkJ¯Y@ÓÆØA/@ à"ªÇ¿ìD]|i¿ãèPÔXÝ<¿Ñ»:X–o¿ìànà]xVAGNbcuPMN J1008-2912?ï–sµþÖ;?•lI'Ã,?Šc€Jq‡?•lI'Ã,?ï®0cõ!?†ˆ'-…?"sç¹·ø?†ˆ'-†?íE(Ø4a?¬½ËË=ó?µÖ¹>\÷?¬½ËË=ô?ïÁ#ç:É?yÒ$ˆòû?nb¹?yÒ$ˆòþ3FGL J1009.0-3137@p®…×E@3¥Ð]óÑÀ9¾~ÝU±À;jõ2F¤)¿ò\ªÈÀù…@BN¨Ú@ÈŸ~µé¿Ë×íÇïz¿èn[ø¿ã=;þ¿àáH2¯æÉAGNbcuPKS 1006-313?ïê=½Æ-?p(îSÌs?eÂB9øÒr?p(îSÌs!?ï¿ÜëFû?£"·ÏË/?€Å.Š?£"·ÏË0?îÑÌq`ñ?¢âÝw€Z?¯2ã8éðæ?¢âÝw€Z?ï屩6?r@jîÿI?jNúçVÉÉ?r@jîÿK3FGL J1010.2-3120@p®Ñ`4P@4
Z?çvœÀ9˜
¨_/À;"30®ô¿Íš ;@ÔΎmìm?ù8}_|<g¿ï–`p?ØÝ|v·Ü¿±ëSBÃ#¿Ð9o•í›AGNbll1RXS J101015.9-311909?ïÿœ€ž
?6ŒâSHÒ?ßØ}=R?6ŒâSI`?ïÝ	vGÅ?|9‹)k÷3?q{DÜz"?|9‹)k÷6?ïp`˃D?—-Y$<¬?'óýf—‡?—-Y$<«?ïý±åš?6Ì:øîÆ?2wè×ë<è?6Ì:øî˜3FGL J1010.8-0158@nl»À n @DÏPßìdBÀ:+î^íÌ!À;ÓN+>?ÀU¤)ó÷è@⧊Hò@	4¿zSÙ¿ãè(b}V¿æ!\?µ¼T¿ävÌsP¿è4í™1PAGNfsrqPKS 1008-01?ïþo²+6á?.²˜êã­?)ÝL'Ü?.²˜êãO?ï}Þ°ŒÀJ?"±*×r–ž?D)îgöÈ?"±*×r–?ïÊ"CÖB?{Š'…¶^ž?zîÞüßA?{Š'…¶^ž?
ñ_?€Ø!Weªs?ŽÒ½Cº¨J?€Ø!Weªr3FGL J1012.0-4235@q#,ÿ§ël@&kþ>^à`À9ž9Pƒ¦À;…§ÉÞ?ôŸ^<vRî@
9""Ï°W@9nà2…8¿íytí<Ú?Üÿ<ÊûU:¿á~ˆ²S[¿î
Š°Ù¸TPSRpsrPSR J1012-42?ˆëº{»ä?‰õÞj"-?ïœQ°?‰õÞj"-?"7h-"'$?´ÇDЕé?ïfD¾"^È?´ÇDЕé?ƸŒ½«Ú•?³J܉'ä£?êQÜЕ	[?³J܉'ä£?«Ã¨ZSK?Ÿ›l7¶E?îCÇ%zZË?Ÿ›l7¶E3FGL J1012.2+0631@mE:Kâ@G?µ!µÀ9¥"÷si"À;"ÿ·¿ÔGpõê @ +Dý5@›{Q^—¿åρZ]™Ž¿ãþ À'¿â©W'Á–Á¿Ô@ßu"AGNbllNRAO 350?ïüêâ-TŸ?<@6Î)1?8¨î•[?<@6Î)1w?ï¤çri1E?"Bô¶Åu?†Æ#e³®?"Bô¶Åu?ï²NnVäC?ƒ
ŽQ¢µR?ƒldjFïR?ƒ
ŽQ¢µR?ïæת
´Ï?a¤>:9ûv?i(UòK0ò?a¤>:9ûv3FGL J1012.6+2439@iøn «†@K+|à%o%À8=†Ñ™»À;S=Êeê@?÷¨¤&æI@WƒsèZ@ïJݤ¿Þ;:žaw¿ä.ŸJç¿åؼUl¿ìК›»÷AGNfsrqMG2 J101241+2439?ï‰|Á'?˜Eïyڌc?Ÿ\nÐgÛ?˜Eïyڌc?ïÂàí[œ]?ˆxٜ ]?~‰R1ÐÇ?ˆxٜ ]?è÷n´]Âm?¯dòj9?Ì"E.ˆöN?¯dòj:?ï÷+"ýàø?P¥³ôQ"³?Q¨ö>?P¥³ôQ"¸3FGL J1012.7+4229@fԀu@K3N?þó'À:r±ÎCÅÀ;¨¬¥åØ7¿âb¡Úà%@]lWA/u?ú‰ ¨+®¿çþ¶lÛ¿ãñðPh+¿ÂOw݇/¿Ó´í¡ÈVAGNbllB3 1009+427?ïÿ/µ'sù?!µ˜'¡\¡?	[	8?!µ˜'¡\u?ïÂ7½¦%k?Šõ$ò¥¥—?~ä!,íK"?Šõ$ò¥¥"?ïÏ0aöte?ys[²†î\?xgÏÅÎb?ys[²†îR?ïüÿ*ý?9_‰ó¤?8f¯,?9_‰óš3FGL J1013.5+3440@g̸`™Ë@KÃC hÀ´À9Á/¡®;À;ÐsۍZ¿çنO@  ïX=@þ¸ Bj´¿áLã1£¿êt@;%è>¿à
ù¼«'È¿ïûàˆìMFAGNfsrqOL 318?ïýVN"ð?7…,†Å"?5MŽèÆ-?7…,†Åf?ï|D%'2?–Ÿ©R·Ç?wp[©?–Ÿ©R·È?ïvډ‡K?‰‰›4vî?'<¤®Ïn?‰‰›4vì?ïÜ^ž
Ñ÷?prè*Rþ?qаùœ?prè*Rÿ3FGL J1014.2+4115@f\ÍÓØ@Kwÿ´€¦À:a)ë‹ÔµÀ<‡ð#éê¿ÜÅèéMY@æ?Ns@c¥ÀnoŸ¿¼UÙü5E1¿åìÖÔà!¿âì/a¨¢²¿éKÍ&¯AGNbcuGB6 J1014+4112?ïÖAUUø?"u¿("…?tßrUU¢?"u¿("†?ïSgð¨M?¥ƒ€
»e?µ"êö]?¥ƒ€
»e?íM£¹`ë4?¤Ûp	"zÃ?µ'â4ø¦a?¤Ûp	"zÄ?ï"i]pÝ?‡O®Ò3À#?Žå¨º#ÈÕ?‡O®Ò3À!3FGL J1015.0+4925@d±?Ýe¡@J[‰€Fâ=À7%cèä÷À:5›Jt?ì"$áûvó@э7`"j?ýU®€0'î¿ÚªðåÁ÷m¿ÚÔm®6è'¿ÜŽHõ¿ÙãÔåŽÔ]AGNbll1H 1013+498?ïò²½ã?cÕU™2ñý?Zš…Ì8ÆO?cÕU™2ò?ïe'>E°_?™ÇGsGX?"O¸7Iô?™ÇGsGX?î¿úÂoXÉ?œÃ÷¶ÎŽÇ?¤SÙ
s?œÃ÷¶ÎŽÇ?í…/;4¿?¨SN,ìö?³×Ɔ&Z?¨SN,ìö3FGL J1015.2-4512@qC$ÜY2@"ÊÊërªÀ9î"
>À;•¹Ù«¡Àð'äÄeJ@‰ý²rÙf@é4Â='¿áSó:¿à
sÒEí'<|T‡?×ރi½šAGNbcuPMN J1014-4508?ïSϞüb?–`0ÞvtJ?•Ÿ s¼?–`0ÞvtJ?ïâÇ÷a?yñZGf?mü8žôJ?yñZGf?íÊݏ²ˆ÷?¤®—	t³?±©'k¸C?¤®—	t³?ïÿý`M1Ë>Æå;¥.>´ý–q¨jß>Æå;¥ˆ3FGL J1016.0+0513@mb€'،@GƒüõŠÀ8K¯é(À;)€,?çAÎüýÂ
@@–Ì_¿ƒ@õß_÷av¿á°à.m?¿å»WeÜA¤¿Ü÷¹èø¿ãw×èè>÷AGNfsrqTXS 1013+054?ïÿgmí«?
°@5?RBJ ©?
°@5Á?ï½nhu#Ã?ŠÖŸ¦ø?€¤eâ·à?ŠÖŸ¦÷?ïÅÙÁ¾¦è?~õÛBG?} ¬Œm?~õÛBE?ïýã½{–?3H<d*·?7hâ#Bk?3H<d*¾3FGL J1016.0-0635@o"ddIV@CÂb¿è¸¼À:A/)¹6îÀ;ÐìwŒÿ?é˜O·Î8@6§µ\™@Z]ÿ—¸?ŒóžGÔ*¿æ*[—ö¿íK£'è¿ïÿ°FP¾¬AGNbcuNVSS J101626-063624?¾ö?ŽNð›?‰8"Ð{Âx?ŽNð™?ᨏŽ9sç?Ðõ‹âuKé?Ü®àã0?Ðõ‹âuKé?ë*U¯¬9ä?°
ôy(Z?ÃV©AOo?°
ôy(Y?ÓÃð·?½ÜλÂh2?æqõž¤€?½ÜλÂh33FGL J1016.1+5555@c'7¼]ê@I' ("tÀ9ÿÓ3[AÀ<Š7üÇ?'Ž»Á¢ý@×`Ô+:ì@3Úÿ•võ¿ä>"èÚÊf¿ç>y|1˜˜¿ãW{¥ÎíJ¿ïÿÍ&}±öAGNbcuTXS 1012+560?ïý"~ùß?=œ:8ś›?3_<1‰?=œ:8ś´?îtäȏ¹ß?«Ÿ%%«ª?¨±³wañ?«Ÿ%%«ª?ï‹5ªÊÑ?×íªks¸?2•~K•?×íªks¹?îë …%?•€o})?¡Mþ'¨
¬?•€o}(3FGL J1016.3-5858@qÁUÿæՍ¿þMV¾|'À7s­uïpÀ9¢ì,
¥?û&…}'âž@¼œ®L9@GÔJDœ½¿á¡—Ú§¬¿àÒ¡'Ïe¿æB°ÊkQ:¿ìU}ÃOJ–PSRPSRPSR J1016-5857?2|­û›ßV?'ØÑÚÊ×Ë?ïý°j@Œ"?'ØÑÚÊ×Ë?[ܚ†àF?rB¯‰'È\?ïò²¼þ?rB¯‰'È\?Ã©)ù?ˆžÃÛ÷;?ïyザ·'?ˆžÃÛ÷>?"î^»s²x?‰>lŠÃ?ïX
$bm?‰>lŠÃ3FGL J1018.1+1904@k1  ôØ@Jýb¿è¸¼À9³e·ýäÀ;§'ûç2¿ìŽøjNAE@ؾoçÄu?ÿ¼Á¿}ƒä¿ç2lw*6"¿×ׂÍ2¿ãøãÊ¿²ïæéiÍAGNbllNVSS J101808+190614?ïú»IEÝÄ?Ou`¾é{?EÚèˆó¯?Ou`¾ék?ïÁ€0Mð?Šny›TÏ?s¿çÙù?Šny›TÏ?¦¹™Ž?†!«Ÿ'?ˆQQ™œn?†!«Ÿ'?ïþI˜¡U+?+è'íñª+?+fuê­If?+è'íñ©Á3FGL J1018.3+3542@gŽï€Uûµ@L:. &{•À:,G"GÛÀ;ç¥b$¸F?â³Ôœ±d@äDó¤ýÑ@d'Ÿ¥!b¿åŠº3 žú¿çë}®ùÊ~¿åË©tX¿ïþq|ýAGNfsrqB2 1015+35B?ïÿ›WàVâ?ùƒ@xœV?	*êG˽?ùƒ@x›¨?ï5¤Må½×?¡JELÁö?™KvCHDò?¡JELÁ÷?ïžV{~3?†	$ÛÖ)I?ˆja \³)?†	$ÛÖ)H?îa9!ºõ ?šogŒÙ?©ìmäP­ö?šogŒÚ3FGL J1018.4-3119@pÆp_®¼A@5!@ÂgïÀ9€÷¹à`þÀ;ëg†ù?ðzÁDXt‹@¤æÛkÌ@D…ßÓdÁ¿Ú̆žó©8¿èsá".c¿ëT³Ý¬\Ú¿ïôf¶1C´AGNfsrqPKS 1016-311?í{d‹#/?·>'5‹àU?´$ßææ†?·>'5‹àU?ã³ùÜðx?Ëåõ<ԙ;?ؘFÃ?Ëåõ<ԙ;?çÉHFÔ,?¸‡ªÊzÕ¾?ÐmorW§Ô?¸‡ªÊzÕ¾?Òkš:í4¢?¯œ¬å¼r?æÊ2â‰e®?¯œ¬å¼r3FGL J1018.5+0530@m–/IŒ;@GÙUÿæՍÀ9V‰µöÇrÀ;S 'àð?ñêâצ°@l"6Ûß@ΓÏ,?îMKMV9¿ã ó粛¿èk¡—ÐýÅ¿ä}å-AGNfsrqTXS 1015+057?å^vHµß?Í -†¬Ý?ÕCoԔA?Í -†¬Þ?ëEcHŒ•?É˒
¤o?Âêrݽͬ?É˒
¤o?å$É'ƒ0?µ–s®þ
Ö?Õý¶m°ù¡?µ–s®þ
Ö?ÞÇ@-¨?Ž'Õ:²?àœusßé,?Ž'Õ:²3FGL J1018.8+5913@bî´ßݵ@HJa€M˜9À:ilØ{À<&¿è+οñ~:Ãu`@ȈD‡™@¹,?Î÷õ¿å›Z—ŽI¿âYl"=·¿Þ^…Ø'Ê¿Øó†FÍç!AGNbllTXS 1015+594?ïô,¥¤$0?€0q0×8¼?W¦´··žD?€0q0×8¼?ïÀè'×¢r?ˆÒÓzz"?‹·.ÇZ?ˆÒÓzz"?îð)Cú?¡á=éÌh? ýn»Æ ]?¡á=éÌh?ïþ²OÉÊ?%X÷Ä0ÞÎ?$Þkcpý?%X÷Ä0Þ3FGL J1018.9-5856@qŞ 3玿û
¬RÐÝÀ6ϽBNÀ9'¤g¡Ð@lá//m@
ô܄¥Á›@òƒë‡x¿Ù£ôüÁ²¿å¯íÎ¥!¿ç¶%÷
ø¿íTš\78OTHERHMB1FGL J1018.6-5856?@}Ç®7B?@¦S-=~?ïûàŽr/?@¦S-=~? §§©SÂÅ?@ƒÜI-`ê?ïþõ……jÅ?@ƒÜI-`ê? "4@á?›$V-½û,?îýÞì»ñð?›$V-½û/?§|We¤?çh³eßD?ïÿ½b¢j?çh³eßD3FGL J1020.0-5749@q½ž 3玿åeSßÙ¢|À7¼ií£ùÀ9Ñޜ)¦?ñØ$ ñ')@Ý‰ˆk@¦nmXž¿—?¨®×»¶¿ç¶®t¿g¿ä1yðºp\¿éc`!¢½PSRPSRPSR J1019-5749?Êü+'@?nj;:Kœ?éõ?[°?nj;:Kœ?ØÕâFTÒ,?ÔHkÙ³…²?ã•ÜՖê?ÔHkÙ³…²?Öñƒ½{?¹Â@ û
?ä‡>!þD?¹Â@ û	?áõ ûÙL?Âß,³a?Ü¿öMg?Âß,³a3FGL J1020.0+6323@bK^?»×²@G"_£Ô†À:+)­xs¯À<ìÀˆì?ëó0Ùç'v@
c~Ì
à@Kø`îW?î×·¿D=¿ä^häq¿êY4ð¿ä|#È9ȬAGNbllGB6 J1019+6319?æΝ+í?Ñ­Deր?ÓöcÞŨ&?Ñ­Deր?ãõjª°l?ÔhljRÁ?Ø*ટ&?ÔhljRÀ?çu^Q_?»!³t"¢ó?ÑCÙ]Aü?»!³t"¢ó?Óu‰¡.h?Ãà§'7ž?æE;q¯hÌ?Ãà§'7ž3FGL J1021.8+8023@`@Iÿ'ò¶@AKg€AÙ¿À9é-¡"ú×À;ù/À·ë"?êÀû1Ühn@_ih¤Y;@!@—tѿ吒fõW…¿ç—nµÚ¿ß9,"ç
ï¿ïÿ±žs.AGNbcuNVSS J102201+802350?ì¡QÕ\Ø?¾·áˆ?ºõsUB?¾·áˆ?¼o[0F »?Æ.ß?ìr™÷;è?Æ.ß?è©A'?µ' k'õ?ÍZû"Õ'?µ' k'õ?Ãí¢Ì ¦4?²ŒË1¦´?ë—L×Ös?²ŒË1¦´3FGL J1022.3-4234@q<‡¿çáü@(š"ÿ%ÀÀ:Au}Zž²À;¦ÝÉtR¸¿æ¼ ÜGØË@Q®Ÿð¡@° M¼¿é‡wÏU¤]¿ãÓ?
_ˆ¿ãn,\€¿í¬"Ç
Ò'AGNbcuPMN J1022-4232?ïS–AÔj?¦GöX?•=År¶?¦GöX?ï¸H•†ò?‰'û»·=ª?íøžCC?‰'û»·=ª?ëߜs?®T(7éM?À›†3Ñ?®T(7éO?ïÆ+ïv?~ÐQ|¹×Ø?|ósjDˆ?~ÐQ|¹×Õ3FGL J1022.8-0113@n¨Äê@F0³ß•ý-À9#a.AÀ;p×%+3?èp/¡òóA@-hì'°ô?ýþjaÐp¿æ—ÿW?ˆ]Úü^ݿ׈ô'Q¿äö­Þl~ÑAGNbllRX J1022.7-0112?ï–—'nI?‹­'&»|7?Šy¤m‰?‹­'&»|8?ìûs$TE?¼1Îí˜þ?¿h$fÝ]Ó?¼1Îí˜þ?î·yɪ­?– ëD^ÓX?¤ˆn#eU&?– ëD^ÓW?çáéE«‡Ý?²þŠJ˜3d?Ð<-t¨ðG?²þŠJ˜3d3FGL J1023.1+3952@f—|€"Þ@LlØà†8À9ßZ"‹ECÀ;䇀'a—?âk¬D}C´@~P¿54•@ÎÇà(õ¿å£€¢Ÿ5¿ëËåŠø†¿ïþ¥l-:?ïȧèMAGNfsrq4C +40.25?ïÿÁéî,÷?Öî@Z;>ÿé"Wç?Öî@Z<®?ïÁ/4'p?ŒñSñúþ?he¶ÇþK?ŒñSñú?ï†Þ»{ù?ˆ'RýT8ž?ŽH{Q!î?ˆ'RýT8›?ïût¬¢:ò?Q™gvœ[è?B-Mw2
?Q™gvœ[ò3FGL J1023.1-5745@qÂÉ?¯Bx¿Ù2ÿÔ™À6¢0'åøÀ9…{2¦Ez@Ïnc¨@܄¥Á›?ýp؍JUå?ìõÒL–S¿â#N+\$C¿çæ+¿1¿Ò¿ì:Õ_â¥PSRPSRLAT PSR J1023-5746?>£,…ò`?=è©õç°?ïü+šoAµ?=è©õç°?%ä*Û°m?B'­X™S?ïþ¯q½RF?B'­X™R?ua¬˜½L?iâù;Ï?ïÕû<¦Î…?iâù;µ?@Ö⸸??x*®PU?ïûÊG¹Ò??x*®PU3FGL J1023.7+3000@hÞeÀ¹™@LËèÀHZÀ:‰'³ò
tÀ;Ü&¯—1à¿ÉæM:<ß@
cäz=ˆÍ?ûîþ?áll¿è㎘';4¿å‰}AR¿ÀYå4ÞÀ&¿Ò§¶|d'AGNbllRX J1023.6+3001?ïýÃ	×·¦?3''Ã\ï¬?1ç±BBÍ)?3''Ã\ï®?ﰌÛIo?wŠï²—Ë?ƒÜÉ-¤<"?wŠï²—Ê?ï­XzÈ?Þaþ†D?"©á[Íýê?Þaþ†DŠ?ïì"
͊?`ïè=òÐ)?cúlõ2vó?`ïè=òÐ(3FGL J1023.9-4335@qIo@_k @':¢?ZˆãÀ8Ȕ¤gRõÀ;ìþ›{ò?Åëô
3î@¶b®ËÚß?üŸ[à{€T?Ülä¸Y¿ß]"–Ž]¿ÝZYOº¿µZeÞùlŠAGNbllRX J1023.9-4336?ïá=èY?kŠÂêèn?nÂèú§?kŠÂêèo?ïÐOàq¦H?"GS$°ÌÅ?wØÇ,ܖ?"GS$°ÌÅ?ïC³Ù¼ìœ?'æËe×Ãy?—‰"Èblƒ?'æËe×Ãu?ïÆ`©"?w€‰¨Ï€?|òO«=ûª?w€‰¨Ï}3FGL J1024.1-3232@pãrà\̊@4Ðï 6kÍÀ8¡ÃPLH®À;uÝæЄ?ó•xÕ©À-@¦mV½@¦L A©n¿äŠ«Áå=¿çž9='A§¿çŒ¶@],¿æ::×þjeAGNfsrqPKS 1021-323?ïý5ª&p?4'ü9Ýq?6R®Ì{õN?4'ü9݅?ïԞý¡~?'«17F?u°÷/Ae?'«17G?ï@:UIë?'õŸ~¾?—øµ]–ª?'õŸ~½?ïÐ<Kèö?pûšü_F—?wáÚ"ôY?pûšü_F˜3FGL J1024.6-0718@ouÛߏG0@DB+ ?:¨À:Z÷xr¥À<J§Å¬G?ù	ùé-@5ò1
d?絫ºrF¿íqTsD‡?êÜiÔ¿èABah>¿ïÿ­µ/w<PSRPSRPSR J1024-0719?ÃüìÀ˜°ý?ÎbËé7e~?ëÄÏÙÓÂ?ÎbËé7e~?‡8)W,RI?šFu©Éï$?ï£Z£N¸?šFu©Éï%?ԒR^('?¸	m
?å¶ÖôPë¾?¸	m
?¢ëJB†â¤?¢•±Z°Ò?îÑK[ב×?¢•±Z°Ò3FGL J1024.8+0105@ngààëgÃ@G$:`NqÀ9Ýë˕•(À;¹ÀI0Ëz?ïcV†Ê_	@
ª£¶~â@d±€9"¿à'…gÏ¿èåÍ-}¿ìK9ðø·H¿ãöÉï!áAGNbcuPMN J1024+0056?뵡¢.ƒþ?ÁcÓèÊ»•?Á)ywEð?ÁcÓèÊ»•?èOºhÌØ?ÑÊN¨»b?ÎÁ\̟Î?ÑÊN¨»b?é_UQ3yo?´¬x,?ʂª»2E?´¬x,?ÍÅIï:L?¿ ºtõÚ?莭¹Ä1l?¿ ºtõÚ3FGL J1025.1+2333@jZe>‰©@LoüõŠÀ:"ÜޓÀ;ã÷YhQ"¿ºþãA@ÉAÂUP@™ †¿åÞ¡ï\!r¿ìqz@¸Ø¿­xÕ~]d¿ì{¡ß8_BAGNbllMG2 J102456+2332?ïÕ'"´ì?'¸Âé,?ux6½¥Š6?'¸Âé+?îö©o¶?¥g>c,'˜? •no™¦?¥g>c,'—?îÈg6ø?œ-_ÇÀ?£yŒ~®´?œ-_Ǿ?ï]š1l1?"`ÙøX›@?"L¹ÏÒyè?"`ÙøX›@3FGL J1026.4-8542@r®€{»bÀ7¥pà<ìÀ9Q½‹ç)À;}«Âßä¿åtªÊ¢Ò@
×á°ß†c@\à*͉¿å€4$Â#ž¿âB÷ÑÕ¿Ù[$_AY¿Ý»‰-±éAGNbllPKS 1029-85?ïù7#w?Dìx7h?K#r#•l?Dìx7^?ïÕ{ª¡·?€áÈB¸K?uB*¯y£'?€áÈB¸N?ïaÏSc¸q?‹†fD3â»?"Æ"ˆñÆ?‹†fD3â¸?ïè&»–:(?aè)'O?gÙDiÅ×T?aè)'P3FGL J1026.5+7423@`ØÑ Äe@Cœ¦ßÓ9ÎÀ:Nd!À;ˆºô]4Ž¿Ý·P‡4šÅ@´A€}é»@•= t.¿èΙ«7¿ìó?ôüZž¿Ä
‰d‡¿çÍRh؆"AGNbcuGB6 J1027+7428?ïÿ¤/èÜ? °û¶Õ¯¸?ËzäxÇ? °û¶Õ¯£?´œÙ?–9ë–ÖL|?ŒÙØÛɵ?–9ë–ÖL{?ï£že0°?'¨»'—:›?‡<Øf³Ô?'¨»'—:–?ïå16!{ï?iB­èHÍ?jÎÉބÄ?iB­èHÑ3FGL J1026.9-1750@pNÔ@(äü@@\ßÔçNÀ8Ÿ–/ÍËÀ;,WvßZ?߶ÞÓ#lÛ@}ÙõI?þ·ÖÁañ¿à]ý<½[ҿ܀¯õó¾¿Ý!+‰E¹s¿Ùo¸ÕOAGNbll1RXS J102658.5-174905?ïþKKƒ="?*ó‰ÎӍ
?+KGÌ-џ?*ó‰ÎӍ
?ïÔ¼ùùÜ?€ä¼ÈÙS?u¡ƒ|k?€ä¼ÈÙR?﯆(¢?€÷'Ÿ¸ƒ4?";¹^u×y?€÷'Ÿ¸ƒ7?ïòC´ßʸ?QŠÔ€êß?[x–@jŽA?QŠÔ€êß	3FGL J1027.0+0609@m·±~þá@Hç3çüÔÀ:\øÍØÀ;ÓÐJ/Îû?×°ý˜G@¤H"Xšv@¿¯ß/j¿ïòýý¶?ÍHਿ犋¸k¨¿Ðqþ4£Ë¢AGNbllNVSS J102703+060934?ËÔEJ?•¼nnqËé?‹"
?•¼nnqËé?ï* 1Ó¯*?¢BtHžF7?š»ùŊß?¢BtHžF8?îtT e_?¡ë4¦I¦…?¨·
½ùª?¡ë4¦I¦†?îÖ}ß?ž¦Ÿ'Çtf?§âžx"'?ž¦Ÿ'Çtg3FGL J1027.7+6316@b6@ Ç@G€8_ÂÞ7À:s­]èÀ<)Ó8 Ù¿Ü­öaµkv@…¤ƒWÛ?ÿïkˆ±j¿ë¹²œR¿ØØ>ÚJ'°¿Õس#È ¿äÑ©u¯¯†AGNbllRX J1027.4+6317?ïîÓ®Ïrß?iT¡"ñ³?a,Q0Ï?iT¡"ñµ?îs:˜ÚÝî?²QÒ!R?¨ÌVrR!#?²QÒ!R?ï9N+BR?•©
0s?˜Ö:wµ»?•©
0t?ï_;±Ye?IdzH¦ì?"‰ÔߓI?IdzH¦ì3FGL J1028.0+1829@k}ì_9K{@Kýfàé´À:_—+*P6À;ìRb£cG¿ù÷aüt	@Ǚ³oق@ä]_šÊ¿Öž?ý'3¿è;h³Ÿ_¿ßåå¼þy¿ÕÚÊPñŠAGNbcuGB6 J1027+1831?ïüþâ¼ÿª?Cwh˜O?8ꩺ?Cwh˜E?ïÈ´‹D8?‰»T"™Âp?{¥º]ãôÃ?‰»T"™Âq?ïD¦×-<?–žíÝ×ôÜ?œ×k%X`?–žíÝ×ôÝ?ïÿŸJÀ?7ÖÛRÜj?-y~u?7ÖÛRÜÀ3FGL J1028.4-5819@qÑÆø¿ßµÿÿ˜ìÀ6ØSéŒ À9Ï´ÂêÌ@yuòËd@1<¸íó@®†‡C*Í¿É#»j"‹|¿á̈&œ'¿åé7ðS²¿ëÂθŸOPSRPSRPSR J1028-5819?fN|ÒëV?p4"þ›?ï鱃-d?p4"þ›?$KކZ°Œ?Cü¬šµt?ïþ»BšV?Cü¬šµt?'ÙÖ¶¹Ø?š)Ÿ°Åý?ïi1O2J1?š)Ÿ°Åù?,ÓãÓjì?&®'«¡?ïþ>'ÁÂÉ?&®'«¡3FGL J1028.5-0235@oN ‰ãC@FD!?ë¨ZÀ:^ÖÒ	L°À;՞¢ŸÓ¿Ü=ȋR6·@½;¾	;@9Nª¿àÛµ7QGh¿çü4Œ'7†¿áðzŸß¿çp¹Ô«*AGNfsrqPMN J1028-0237?ïÿ搝>꒞0QÇ>éoøb䢉>꒞0X?ï®ÃÇÁO?&PÞ|N?"O¬>½?&PÞ|L?K«Dz?ˆ¥'Ã*-?‰-.áw?ˆ¥'Ã*,?ïø>°:±Ã?Hõdí<š?O?8øÒ?Hõdí<ž3FGL J1030.4-2030@pz-••@?eþßnÀ9¤ºB†MÀ;~o09ƒ¯¿µ*ÍóŽ8°@´ìL™á"?þ;bŸ1‰¿ã
]Nd¼î¿àÕAêáÇ¿Î?©˜5Á¿àkÎZXAGNbcuNVSS J103040-203032?ïý†ýÒ?9"êy³¿8?73Ïào/?9"êy³¾Ù?ï̞£LHA?€ÅRj÷ˆp?y°®YÛ߬?€ÅRj÷ˆq?ïÏiØ{Ïà?wx0ŸËJ–?xKÂÒ?wx0ŸËJ"?ïãþ[Â%F?c¹¾Îï ?l¤=ÚºO?c¹¾Îï3FGL J1031.2+5053@d.%¿­@K7èÀHZÀ94
ƒvA¦À;UÊÆbP¿ò–i¹W$@áë#$j?ûHŠàï§?²ïâ{ŠºÚ¿âÝoFVH¿ÒñŽÈá¿Ífl_hŠAGNbll1ES 1028+511?ïï!k€³?b¨SðÛiD?`ޔåM*?b¨SðÛiG?ïÁ,/œ®?ˆOŒ̎\?iè1¨¹p?ˆOŒ̎\?ïiäLÅÂ?ŠhÿªZ?'Ãv}çGØ?Šhÿª]?ïýZ›ƒ¨?BÉýλ?5+#⿊â?BÉýΠ3FGL J1031.6+6021@b"àç6@H›¿çáüÀ95?VW$ªÀ;UøZ?Ç% þä@	1í]ç@	?n)ÿ¿è˜ùX›øo¿çpØæi3©¿ÞµÕ
|Ú
¿í/ö‡,AGNfsrqTXS 1028+605?ïùÎnȑ¼?Q¶o`N¥µ?HÆDݹ?Q¶o`N¥³?ï«ù+è7?Ã&íPÏ?…µò??Ã&íPÎ?ïY'ý¾=?–‡'v´jÂ?ŸÔÛH8?–‡'v´jÁ?ïÞ-ŠÕ?içs­­Jå?pé~þ:•I?içs­­Jà3FGL J1032.5+6623@a»/ÀL‹Ê@F¦>ÿðÈÀ:ìÕy(
À<MiŠÞô¿Çæ²üìû@A'Ž³6¤@2o¿¨Í¿êÚԊ¹àj¿ÛâîwAý¿åþR—¿ÝÀÖw¤	AGNbllSDSS J103239.06+662323.2?í>
äoû?À¶/)íÐç?¶¨ß€(?À¶/)íÐç?ïNÐ#ÚG¥?¡åøCV?–%û"·f?¡åøCV?ìÂàÿ²Cû?±5©‰)!?¹èømà.?±5©‰)"?ïª*ï''?ßv¹â,?…uD6:va?ßv¹â-3FGL J1032.7+3735@g
Âß
A1@M‡9á£À9A§~^ª°À;ʒ~e'¿í!ìè0"@Rk~SB@™÷?':¿äìðgAéÁ¿å*<éâ©¥¿âX<'ß©/¿ä²T²ERAGNbllB3 1029+378?ïëMH
D;?eŸ+˜~oÆ?d²·õ»Ã|?eŸ+˜~oÊ?ï
å|d"Æ?¨ì˜iÙ%á?ž£Psmg7?¨ì˜iÙ%à?îÆӉ>–ª?–äî1á?£'Çl•Z?–äî1á?ï¬9ܲ?…8]rœ",?"ñˆÓ\º_?…8]rœ"-3FGL J1033.2+4116@f+zß.Ï @M2R¿ÀtÐÀ8áî¯u£ñÀ;·uª§?ÖLž?Vé,@à Áìt@'Ð pË¿ßa£½‰ä¿çB‡ÜOC¿à<%ÿ²Áø¿ì#ٍiNgAGNfsrqS4 1030+41?ïørS}ô?QŸ$IRª?N6²Ü/?QŸ$IRª?ïd/ôJ?—ñÞ'Èg?"zAvÀ?—ñÞ'Èh?î˗m7x?šãúCóî?£F¹,ˆŽ?šãúCóí?ïZ1y1Á‰?ˆwo7n{?"¹ÐÙÇÎÜ?ˆwo7n{3FGL J1033.8+6051@bxæÿ}ú@HŒö@c^À7Ç9k[˜­À:Ñ«ì'tº?úy4I]Áý@æ~ZÎؖ?ÿļ'ÂåÿÙ蘙®+;¿âÛÆT¸"¿ä qFŒ¿èjó®AGNFSRQS4 1030+61?ïêy£$]a?odŸÜÜ?e†\Û¢e?odŸÜÜ?︯Ï
mé?ŽLSc¦J?Ô=d†?ŽLSc¦K?ì¸hüŕ?¦à1"³Ð?º?ü¸Ó^?¦à1"³Ñ?ïþ½5ƒ.!?,n¿õ¤z|?$,§Íû¤?,n¿õ¤zò3FGL J1035.2+5545@c?ʞõ#-@J/xßå®EÀ:*ôœõn­À;ñ<¼HñÀK|7³ög@Þ/â+Y@‹õ €"Ž¿èe~Ñ[¿¿éöíO×·?¿é«k¿îøË1}bAGNbcuGB6 J1035+5542?ïþ1^ØCÆ?=nà[ž«ƒ?,ê{Éõ?=nà[ž«~?ï¯%Êbð?ŸSî›c?"6gCýî?ŸSî›d?ïBEæ?'t¬Dð\?—·]Ã=ßÜ?'t¬DðZ?ïÿÏËçÚ?
ÄÅãGV>þ8« ?
ÄÅãHK3FGL J1036.0-8317@r®½_ÜßjÀ5O_¹£ûÀ9àG­=»LÀ;®ygÊêt?ê÷6õé@
ùpò[|¨@¤H©hš¿«_QÒ¹(‰¿æL!·hj*¿æö}‡-Ì¿ïÿ-zYPSRpsrPSR J1036-83?뀝·½â?Äa™Q©3?Áýˆõ!x?Äa™Q©3?ÑUî¸È?Ì°9¡S÷?çUþ#›ÿ?Ì°9¡Sö?é-YûÃ?°Ð.Tèàk?ËJšó¹?°Ð.Tèàj?Ъ^‹–™?²f)&´?çªÐº4³s?²f)&´3FGL J1037.0-2934@pî¼ßï¿@@8Ïà0VàÀ9¢<PgÀ;‡vG…?ï­Ýò ,A@δMÏì'@½æ¿Þ}ºüüщ¿èGL'!L£¿äŒgv©!¿ïÿ =Z~AGNfsrqPKS 1034-293?ïýÖ·"ëÂ?3·kþ*<†?1JCØ¡ïÖ?3·kþ*<?îîJÁݎ?¢»©³?¡Sî''$?¢»©³?îXƒ"4e6?žÛÌ],G?ªwǼ¹¬¿?žÛÌ],F?êi!fo?©ª`û7Ö?Æ[ççzfD?©ª`û7Ö3FGL J1037.4-3742@q9Ê?‰'Ë@1òŽ AS‡À:*®í¾´ÜÀ;ÅÌðÞúÍ?ÕêêÞÊj@ä4i>÷@
îßòŒ¿èb^<¿æ/Y^ëô¿ë'lkZŽc¿ïÿ9M(¨AGNfsrqPKS 1034-374?ïÐ$â¯"?€§@ö}?wñ펨o?€§@ö~?ãPò¸™Ö?Ðüôn"øË?Ù_ØŽÌT?Ðüôn"øË?î‡(}…?Ÿz®å
m?¯ç~H'³?Ÿz®å
k?Ø#ôê+gn?½CKøڔ†?ãîŠêLI?½CKøڔ†3FGL J1037.5-2821@päo€Uûµ@9☠uUíÀ93Ád¹½üÀ;€C_?ÒïñŒA9@Õ Û,a@ñºÃ.¾¿æ8÷׬=¥¿åáJ‡°Œ¿é®÷!F¿ä"\@?-AGNfsrqPKS B1035-281?ïþ¸ÚâAð?&4lSˆ_»?$rQÛàìz?&4lSˆ_
?ï¯:µG'B?Œ"UFIF:?"1R®¯Œ?Œ"UFIF:?ï·%Ѥ•?U7ƒ9F?'6‹–ú›?U7ƒ9N?ï\œÒÔ÷ê?‡~AÂ	i@?"le¥a»?‡~AÂ	i@3FGL J1037.5+5711@bùŸ˜=@Iáü`8NüÀ8<ÃÕ­FÀ:èâï?õ.HËùp@¡½Gɘ:?ù!†â-\¿ÓS'¼Ä¿Ü,+³sE®¿Ù[žÔA
¿Þë·V¡öAGNbllGB6 J1037+5711?ïü¯­ÎB–?C·q~&²ê?:''ëM@?C·q~&²ä?ïÀHÛŠ?"u˜DŠd?Œí߉?"u˜DŠd?îR²mÑ[? ÅâJæx·?ªÞÄÙ"êX? ÅâJæx·?îw¡p} ì?—¬B‹L,ç?¨…èø-ñ3?—¬B‹L,ç3FGL J1038.9-5311@q¼ M@·o?ÓՀÀ8-¿¸èzÀ;)iϧr ?úÆbã$''@F5‰ÏÍ@#Qv?Lq¿ã¤˜";¿è@;ªóV¿ë'ÞFz}¿ïþè"IŒwAGNbcuMRC 1036-529?ïï(!î
?]ö±½éåò?`×Þö?]ö±½éåì?ï¶ñºtÑ?"'QäÕl?'C'bù‹ù?"'QäÕm?íåÿh	<?¦'0%c±è?·˜Ð¿¶%?¦'0%c±è?ïõÔâÔÓ?Të™.ö?TV:VYþ?Të™.ó3FGL J1040.4+0615@nXà†8@JE»üÊÀ8Ñ:6\³_À;x§P;¶?éq‰žò@OŒ¼çQˆ@ÏgÀƒ"H¿áø~«E'Z¿ãõ1Tƒ1p¿á÷,̑é¿èÑ2uÚAGNbcuGB6 J1040+0617?ïõԃ'¦ë?|£ð&ÎD?TVøú²*+?|£ð&ÎD?ïKþÀ¸Ì?œRŒp½ºN?–À'èæu?œRŒp½ºO?ï$r°¥½Ã?–kGH
?›q©ëHGÄ?–kGH
?ëÜZ?•6=/\ñ,?¦aB:_Ö?•6=/\ñ,3FGL J1040.8+1342@lÄHS'^@L]⟜èÙÀ:¦–À¡E`À;×Û©¢f?Þ¸4r@–`Þg)?ü(ôÀÜ©?íó™Úç¿îö'LdÌ?ë@"!'÷¿¿Þ «ˆìAGNbcu1RXS J104057.7+134216?ï÷¤²ä?mâ³ïÐ9?Pz¶š7ñ
?mâ³ïÐA?ï¦7ªmYy?"Ò"Z$´Ö?†rd©¡{?"Ò"Z$´Ô?ïAy^£Ö?Ž5r½w*¯?—ÐÔ+å8?Ž5r½w*¬?ïÛÀtñºV?‰MÙ~¡G?rŇ"ÔÉ?‰MÙ~¡G3FGL J1040.9-1205@p<>_·¼@C͆_¡PÀ:_Ü#åHÀ;×m‹ô•i?Ù)EÝô6@s¨(}¢˜@ÚßVø4¿ì	uéªíÄ¿¹e'»ež¿á`!œn¿åÞµ'ƒSAGNbcuNVSS J104108-120332?ïò`KçÀŒ?f[ã!Œ
W?[?h0~ç+?f[ã!Œ
S?ïZ–"6-?j'e›üÈ?"­>í™:"?j'e›üÈ?ï'QÛ¨?ˆ©¡¡ø¯?‹œ«‰?ˆ©¡¡ø¯?îÛ6{Û?"ã$¨s`?¢LŸþ8BP?"ã$¨s`3FGL J1041.8+3901@fšž`=Wy@NGU?ÍuiÀ:Ò2Ò»#WÀ<]€
×Y?âUÁݧÝÌ@
÷œ{?ÿ'dÿ^'?ïþæj­ž¿ÍÀ…¿z²V¿æÙ«<%¿Ü×k\fÖAGNbllB3 1038+392?ï]âA‡Ìá?—98± ?"C·Ïcõ?—98±"?ì%gžâ]ñ?Æ%²EÓ?¾ÔÃíz?Æ%²EÓ?ëþa&QËñ?±XøöZï?À{f¸Ð=?±XøöZï?ã&¾ho÷?Å0`—K à?ÙŲƒ/ ?Å0`—K à3FGL J1042.0-0557@oֆÀ
¡©@F:ØÀ  À:kÃ
0j+À;ÎÃÍIÊN?òi´Ï€t@
Í."®×?ÿr?7£Z¿êﴈ³Bb¿èJWqMl'¿¦ÛnŒ`Ý!¿ßˆùiÊWAGNbcuPMN J1042-0558?ï³½‹"í?'lÌ)Išö?ƒ8·Dq?'lÌ)Išö?À€‹?²×h÷ۗ?¥Îô÷÷A?²×h÷ۗ?ìFµ×2?©îøÓü'/?½ÊQG‡¦i?©îøÓü'.?êQ|-»ð?¿ú°ď?ƺ·IF?¿ú°ď3FGL J1042.1-4126@qf1Ào@.cŠ '§À:˜PÀ;äcâ'§å¿û!tïÁ@b=OçÉ?ÿž/ÀâÞ²¿æÃڈ!L+¿èiòX]ËH?½ž‰`™üI¿åë®ïí
_AGNbcu1RXS J104204.1-412936?ïþÈ|#ž"?$½¼*àï?#x=ÆÌÐ?$½¼*à¶?ïã((ÃßT?w
†¯Žð€?l××< ¬®?w
†¯Žð~?ï͐?Þô¼?x&~ÂÈÚ?y7à…¢j?x&~ÂÈÞ?ïÿÆø3ê?a{~ö7>üƒæ
õªŒ?a{~ö6Ê3FGL J1043.1+2407@jsˆ M@NÝÀ:SÀ9l5Qñd\À;²£á8k?å-ÇêB‡@"iÞ @ðO@Z
=¿ÙÿŸØwûº¿åSâì&Œå¿ä@½€­Ã¿åŠRĝÿ/AGNfsrqB2 1040+24A?îá63ñ‹s?¥–.òu€ƒ?¡ìœÀçHÑ?¥–.òu€ƒ?ìÅô-¤†%?¿m#½‰œÙ?¹Ð^'ÛÎÛ?¿m#½‰œÙ?ìhrvõÄ#?¬ÿô®ßæ?¼¼lHQÞå?¬ÿô®ßæ?ädڃ‹Àf?¼‹K*yp¾?×6Jøè2?¼‹K*yp¾3FGL J1044.4+8058@`I¥Ò@AXe_Ö)mÀ9Àû¦ÔëÀ;\íbnŠ!?î3€FêÜ@™¬Ÿ°´é@"ÀŸAú¿ØEÛpBw
¿ë$¶-ׇD¿ê:` |!d¿ïü9®;VAGNfsrqS5 1039+81?ïýÌï7%?7³ô³qäâ?1˜†GîÙ½?7³ô³qä£?ï1e!݆Ê?¡>­áaEW?™Ó[ÄO&¨?¡>­áaEV?퇻 P¯?¡ÿúAŒ}?³Â&ýŠ'?¡ÿúAŒ}?ëK¡wµ5£?°òf^Ã5?ÂÑz!+)s?°òf^Ã53FGL J1044.5-5737@qé2`o¬`?òx W À6·èɂ•qÀ:BÙ­…ߨ@z—ì¯@aP!«vf@~÷€—:¿ÞÀõ0̯¿äT]ã
%ô¿ç
€û¬Íî¿î‰ÿJÉPSRPSRLAT PSR J1044-5737?<š³u½ç'?=wrÎ}ÖÎ?ïül©'HC?=wrÎ}ÖÍ?&uš9cӉ?C7›Í‹­'?ïþ˜¦\iÁ?C7›Í‹­'?"¯T{DHb?"2´'Ïô ?ïb…\%ݽ?"2´'Ïô¢?-"ÐÂh.«?(–ª:é‹?ïþ&ÂóÙ~?(–ª:éŒ3FGL J1045.1-5941@qù±_ˆü"¿äB% 3ÍÉÀ6´ýÓÕՊÀ9­Õ~L69@z§3
C{@4ü(+?ýÇ3½G¿Ò`x:Ï3Ú¿äÆëvÛÿp¿äˆ§¾öJu¿ç.†%HŽåOTHERBINEta Carinae?¢ƒSؼôî?¼º‡Î±+?î×ÊÂt0°?¼º‡Î±+?AT}¡*kþ?Užú§—Ô÷?ïûªà—µd?Užú§—Ôø?Ñá£ô(ŸÓ?¹/§'ô*j?ç.ë°?¹/§'ô*j?}zT²`Ô?síښñÄy?ïÅV›>X?síښñÄy3FGL J1045.7-2926@q	ÜÆø@9îσ³~À9:kÕ;0XÀ;"'»0?â"Åù/<•@œÈÿåí@¥bYât¿æ(Bn1y¿åÍa1É%οä+RÉGÿj¿ïÿÒ1ª`ÖAGNfsrqPKS B1043-291?ïþ$m¯'Õ?1S¾ø_•?-¹%
''c?1S¾ø_•Q?ïÛ@`˜#?|µÚQ"Å?r_ϳóíŠ?|µÚQ"Å?ïSñåTÿ?"P…×?•œ!ÃU`?"P…×?ïü3»:¥?;Ld…"ö?>gú&*áf?;Ld…"ã3FGL J1046.9-2531@pèÙ'ÿ@=gqß@lØÀ:'8§ç:6À;ÉÙ³eº?ÌW'2_@cü3?ýŠ¿_&?궾ä½ëo¿â]'ÿ´'Ô¿Ä'ÿz㺿¿æJ£Ÿ#h²AGNbllNVSS J104651-253547?ïîpe¦Ì%?eö`D˜r?ašY3ڇ?eö`D˜t?ïqéÒfr?–‹¶¥¿3½?'Âų1¾g?–‹¶¥¿3¼?ïSôç4à?ŒfOŸ5
[?•ccþù?ŒfOŸ5
[?ï(A7ù?"©@É`-?Üº÷Ù?"©@É`-3FGL J1047.6+7240@`׆@ €@DÀ¾ß¤?æÀ9ž.§³7ÐÀ;²Ä§d]x¿ôêeI/ôº@òfsÒ_´@mŽo¿ã~¢zòB0¿á币Õò¿à—í+ð|¿à*'ßB	AGNbllGB6 J1047+7238?ïÿŽs¿V?
jòlEL?c*\hL?
jòlEÁ?ïÄ,ø;ª?‹Ø
÷v3?}éƒâ*ú?‹Ø
÷v4?ïÐþ@›Á?lŽDºx?wÿ€ß²?lŽDº~?ïÿr"¶µ¾?Âq:K&7?­i)HV$?Âq:K&ß3FGL J1047.8-6216@r"ŸºEÀ9µ ÝDÀ8-r)HÀ: †ˆDÝ?öoôǽ™S@í/çú$Ê@<|z¿ãðÒ
¾¿èøò;‹
N¿èrz_'éå¿å3ø·P'¤AGNbcuPMN J1047-6217?ï‡ff‰TÖ?"ý´aqÇO?Ž&f]ªÊo?"ý´aqÇO?ߍkòcdz?Ô7½Ã7 ?à9JÎMÃ?Ô7½Ã7 ?ëLÂRð?°^F"Ñ?Âϔö·¸@?°^F"Ñ?ß­ZfÁ
?À]¨½JmÍ?à)R̟zò?À]¨½JmÍ3FGL J1048.2-5832@qöíÿ'+¿?⏣?Ïg¡À6Sà_PÈoÀ:ü¨\ªü@.¥5¯v@%¼`CÃ@¢ùš
WÈ¿Ô¸…Jµ¹¿á_6›L¿æs7ò#=¿ì8w{ó§"PSRPSRPSR J1048-5832?4'Ì2;š¹?+gÁ`M&?ïýo¦y¸‹?+gÁ`M%?$ÇÐÖL`T??6Ðõ¤jÁ?ïþ³'ò›9??6Ðõ¤jÁ?tn;ýŸ½Å?XA"
¸?ï×#ˆÀ"?XA"
¨?$\˂èýG?$Çpónú?ïþº3GÑo?$Çpónú3FGL J1048.4+7144@`íßý`é@E#,?ùëÀ8ªE¹GµÀ;jä'Ë÷»?ð"……æ^n@hðÎ3Õ@"m`*¸¿âp4؜0D¿å·oK
¿è'µ"9¿æ€¾;x.AGNFSRQS5 1044+71?ï÷Ð)LaÛ?S<$ÁxHr?P_­g<L½?S<$ÁxHb?î…Ý{œ?°jÔ¿M0?§¯B.¨F1?°jÔ¿M0?îŸß%Î=>?˜žH:¦Ð?¦
£,?˜žH:¦Ñ?ìEMAŸ?¯°7csÆà?½Õ•ó/?¯°7csÆà3FGL J1048.6+2338@j¦ôÿ†]}@O/ »èÀ9¹i,êCÖÀ;½WQ­D?ív½µhé4@?mÚÎî@Nvÿ»·|¿¥Ÿj7_¿çÏà0½ô(¿â͉:¦Äû¿íY¡ÃAGNbllNVSS J104900+233821?êk2ßP?Ãf
?O?ÇÆS7°'¼?Ãf
?O?ægMBQT?ʪ9ð¾¡?Ó1eÕ{]Z?ʪ9ð¾¡?æJt?¸ËàRàH?ÓÛkÛÇþ?¸ËàRàH?Ûñ˜'ÅŒ?·bRpÕ?â1·:?·bRpÕ3FGL J1049.8+1425@lÝ¿˜0ä@MË@ÒÎÀ9÷¿µ'À;˺µsô?Õ>vn3@Ëãæ™Òz@¨‰?"O[¿èÈ蘟¿ã€ßxöáÉ¿ã<æü+'³¿ïÿÏ7؀×AGNbcuMG1 J104945+1429?ïúDûbý´?kLíi¸Ô´?Fìt	8 ?kLíi¸Ô´?ï=`vÞ?šß>^cµ?˜]óñ$<'?šß>^c´?îk¨³aÌ&?¡'éõàë0?©EtÉã=­?¡'éõàë.?îØ>#±?•¸\LÊC^?¢|ýÄç?•¸\LÊC^3FGL J1051.4+3941@fMp€0<@OjÀh:|À:s0V	!À;¸Ir9Ù@?Þxš¼ü˜@
—ÉøÜö?ú¡I …[Ÿ¿ïÿëü¨:?ïýøÞp¿ܮ'@òʟ¿x¶0d]ÿAGNbllRBS 0909?ïéf5*)o?gDv¶ivÐ?f™ÊÕ֐?gDv¶ivÐ?ï£\aš?"BO6Þo?‡:hç™}Z?"BO6Þo?ïK.åGf?Ž*ö÷ÑU:?–š#\—H?Ž*ö÷ÑU;?îçêÁMWù?šÍxÖ¢Ê?¡Së*€"?šÍxÖ¢Ê3FGL J1051.5-6517@r-'Ÿì™òÀÐ3³À8ҙ!¤•vÀ:ñÅÒ݈¿¨~".xðI@û)/y?@Äb¦-¿åÜ©ì£ö¿ëú¬{ôm%¿âúðcLM¿àš_ð´AGNbcuPKS 1049-650?ïÊ]hñtÊ?'èJ™Ô?zÑK‡E›,?'èJ™Ô?îZ¥úßN?¸¬SD(!$?®šU R?¸¬SD(!$?íLµ=›¾q?¨¸}»	]?µšV"l?¨¸}»	^?ï@Øàóu
?‰á	\ˆdž?—äãá'^q?‰á	\ˆd3FGL J1051.8+0105@oD  ô×®@I¢¹¿©Î›À:(48ñÀ;¾º•"<¿ôÉ&úë™@¾g'‰«@…n€;N¶?à<LCûWz¿èuzýŽP¿Ñ蛡¿ãÙÝu«A§AGNbllNVSS J105151+010312?ïþRKaÖË?,édæ_Eœ?*ÛIâ"^¦?,édæ_E†?ªn~?–@'+ÊÌv?ˆUd`{D?–@'+ÊÌv?ï"ÙÛB× ?"¿ú
B³'?‹	‰/J8?"¿ú
B³*?ï÷ E‹¹?XŸ(	=?P¿uðè?XŸ(	83FGL J1052.8-3741@qf[@-¹@3uÑÀQ"GÀ:Aµˆ©\À;¼óË>WT¿ûrßsB—Õ@ˆnÙ§{¯?ÿðŠß—¹¿êք4ò>æ¿áž0I@]5¿Ò0¡Ðl6¿Õ-îƒ^wAGNbcuPMN J1053-3743?ïþ|'6€?)w¸=hŠË?/ˆ=Œ—þ?)w¸=hŠ¸?ïÜj4p.?|ÛK"{?qôJåÇé´?|ÛK"}?ïÆ«Cf-?v¡-%D?|ª^Løi:?v¡-%>?ïÿ[i}(?ªhhÇ®?2Ð[*?ªhhÇ­ê3FGL J1053.7+4929@d*à~Zy@MŸä6vÀ9­µ|N/8À;'
ãˆÐôÀ .s±@mwô-cæ?ü»È€aå"¿èˆÂ¬bt¿Ð¹9#¯¿Õ,¯Æ¯¿á}"ð+2AGNbllGB6 J1053+4930?ïþö©ÏǬ?-½Ù"? •c…:É?-½Ù"ñ?ïÐ:´"'?‡¹P?Gü?wâø%î¶ù?‡¹P?Gü?ï"x49?‹ãþ@?Šáòñ›ÿŽ?‹ãþ@?ïÿÒ¾¦§?ÎðQp7>ö þ,­
¼?ÎðQoÝ3FGL J1054.5+2210@k!«`kz¢@O‡@`B_÷À8ÕE!r@À;'°Ql^¿òž"•P‰°@¸'uåµQ@šþ¢Lœ¿äÒÒË?¿ä M¼¿âJˆÝ½=–¿à]Åsù2BAGNbll87GB 105148.6+222705?ïÿ¬…J•?0¼
0aù?þ­Z¬?0¼
0bÄ?ïБÊÒÀK?"Ëä½Þ®?w·–ŸÚ©?"Ëä½Þ¯?ïÑw±°Žö?w1ç«s£?wD''¸…B?w1ç«s¦?ïü'%ßk?Bööã"?;ïѶ?Bööã"
3FGL J1055.8-6025@r*@ºˆ¿æ°ÿðCRÀ8>öJt˜XÀ:0ÞÿÕ7Õ?ÿ¸VÉ}÷@μlØE|?ø¥ˆX‹¿êYÆO°‰¿Ç;šNº"¿å8BhҞÀ¿íú±°=PSRPSRPSR J1055-6028?=óë?7]ïîkÕ÷?ïü]|<?Â?7]ïîkÕ÷?IJÜ˦Û?a£o
7?ïù­HÍH?a£o
7?¬¨û'ÁÚ?¡þ®'ý£?î5pMƒï£?¡þ®'ý¢?"^2u• c?Œw³ªù×?ï]lSRþ?Œw³ªù×3FGL J1057.3-2341@pý8€®@@…ߨq¤À9ܕyyh¢À;·ûêlj—?ôgë†Ì7|@Âó5AU`@ˆàdõ"¿Í¹fb#zr¿ÙŸ
¦¿í~×?'ÄP¿Þ;Ê®d'AGNfsrqPKS B1054-234?å$H'@?ÏÍù©?Õ·ïoÚû?ÏÍù©?íŸ‡"Ç}?ÃT¡úý?·›ÆéÄ?ÃT¡úý?ædÌ'"?¶Ì•–Úwû?Ó6g±»ÜÇ?¶Ì•–Úwû?à¥ûé"#h?į&ÌnÓ?Þ´,×¹1?į&ÌnÓ3FGL J1057.6-2754@q$±Ào@<{Ÿ³À:w•¤A"HÀ;ÌPwؕ¿ãÍç˜ÄÌ@{f°6?þ,TßÖ>æ?èvK6gΤ¿ã%ZºÇοß@‡ë­sҿ̎)‡ý~µAGNbllRX J1057.8-2753?ïú`çm3?G@Ëï*|®?FÌbK5–?G@Ëï*|°?ïÒ9	™¼?'
AR>ô?vðc{3!Ñ?'
AR>ô?ïq´Øžîû?Š'M#<–ø?'Édì" ™?Š'M#<–ö?ïøÀ+Ú8Ù?IB®»´ú?LÿP—?IB®»´ó3FGL J1057.9-5227@qßÔ§e4@"àà*!½À5öU/}ÉÀ:—«bï¹a@JÝð
¿w@nFM—7•?ü,y¦Žu¿¸Ú§MXŶ¿ÜáåÂUê1¿éL)õØðÙ¿ï¥Ó–7óPSRPSRPSR J1057-5226?I×ÎçږÚ?P¡lÏ­å¿?ïùŠF	Z?P¡lÏ­å¿?Qe@`N'?`= ƒK¶€?ï÷Mr_ÏØ?`= ƒK¶€?šÅÀq‰Øë?›0üCÄ?ï)Ñüs±9?›0üCÇ>vRpn´>€eUY|ÞÉ?ïÿÿÓÁÁ\>€eUY|ÞÈ3FGL J1058.1+7010@`ûrà\̊@EÿüŸù/+À9vëg†ùÀ;à±û.·¿ã§|p¾Ùð@Cٗá]¨@ŸÜ TsË¿æçˆûÅ;g¿éO>	X¢¿êùNñˆKœ¿äÆMy'AGNfsrqS5 1053+70?ïûÌ>äÑû?C$Ϩu?@Ïl¸?C$Ϩtþ?ïlÇXz?Ÿ0Fã…'?'gð¬_=?Ÿ0Fã…'
?﫵 É,^?B<øNÐL?…—Í´èt?B<øNÐP?ïÞH l#D?n€.º&%w?pÛ¯Éî]³?n€.º&%w3FGL J1058.4+8112@_ÿ+@öjU@AdË@ÒÎÀ9…Aî·Ù À;u¾¹å?Ù!Ââ,[@NiÔÚã;@T3‰M¿éò«ð"7¿æW˝;©h¿ëx`!ÿêYþQæ7éAGNfsrqS5 1053+81?ïþOu%í?/Ûé¸÷f?/Ë­¡+'?/Ûé¸÷<?ïÍcÙAhÒ?Ü5{Ò?yN_K—??Ü5{Ô?ï›c1Áم?"¦"äZ6w?‰'3‰ž¦?"¦"äZ6v?ï×ô¸°6I?i݊-Ù×?t£§äÛ¼?i݊-ÙÒ3FGL J1058.5+0133@opŒ€A@Jc*`%څÀ7s\#íEÀ:µ#I±#ú?òè³ÍøE÷@Ð>â¾ÑŒ@碥0üw¿àã ïá¿äoÒBW"¿ã•ýmt¿ââ0-¼ž#AGNBLL4C +01.28?ïýëYQ¶?@Çz~p¾?7ø¥5rSp?@Çz~pÂ?ïÃÇ'¦]4?ŠXè"úˆ5?~l,Ñf‰?ŠXè"úˆ5?ïµMöÝå?–f㈲×~?œ©VA$CC?–f㈲ׁ?ïùá"Í>?GYöÄ+Ë?H{w Ëš?GYöÄ+¾3FGL J1058.5-8003@rŸìºËCÀ2G?}ÄQÀ8%ðT'RÀ;*sMÕué?öfnSŤå@Õ	2®¨õ@óaDéi¿ÝÛ³'×hæ¿å¦,áÉ¿ä‰][û©Y¿çØH»/ÛAGNbllPKS 1057-79?ïíÅün?drص¤í?b:ú'o•?drص¤ë?ï°~,ô€?"æ]ºr²?ƒàztÂßê?"æ]ºr±?îÂ쒷1?—Ãêy…ßÇ?£Ñ6Ԏ}?—Ãêy…ßÆ?já?Z#Xãàè?Žšœ;åH
?Z#Xãàè3FGL J1058.6+5627@b³fàé´@K8€iFëÀ7é´[¼¿9À;2¥n¹òÀ  :G¤"@'6MïÍ?ÿ€y¿ß)²_§õ¿à½0o‰z¾¿à;QÈÕ¿¿×'m½@AGNBLLTXS 1055+567?ïÿi¨¦G?a¯aݖ†?Êë=w?a¯aݖ~?ïÊz­Ž˜
?ˆŒlb)H?z©8³ùú?ˆŒlb)G?ïÌÖÞSÇ?¿ÍJu±°?yû"Öã?¿ÍJu±¥?ïÿý²€jä>Ç>º¿ùkÜ>²kü¨â*ÿ>Ç>º¿ù^V3FGL J1059.2-1133@pšÑVŸ@EYá @è(À8AëÒK'À;4]"<?Þr!+û1@ÓrDëíN@qÀa¯r¿Þ¶šm¡e¿ã/ØñÚ^—¿Þ"]
]qÜ¿æîBøFAGNbllPKS B1056-113?ïþ=øÆç?)¸>@2æ?, sž!¤½?)¸>@2åÀ?cbæ?"ß`\z¥Ó?ŠW8ç'Fô?"ß`\z¥Ô?>Šå'?hSu×?€Ø]x†¶,?hSuË?ïɂ~Csä?r
×
3¦?{>ÀÞF?r
×
3¦3FGL J1059.9+2056@k'_ôö@Oî2à'¤À:kUž˜À;µÕЁ3?ê—×p¥ëž@gßbP­@Œh€Z¿éÌ,QÓÃr¿åÈãï(Ah¿î±}cX?é€4
AGNfsrqMG2 J105938+2057?ïý*¤&Ç?7AõPm¹?6ªß~ÉÏ^?7AõPmÕ?ï½ÆŒ†~"?ˆ×Í"(Z—?€Ž\Þ`Zó?ˆ×Í"(Zš?îI#›?œCß´§1?«n=ϦG+?œCß´§4?ﶭÜÛ[?'¶ûõêE•?'TˆÉ)?¢?'¶ûõêE•3FGL J1100.5+4020@eù«ÀãŠ~@OÌÚ`3F~À:
µÙk@ÁÀ;¹u.€F¿ê_hè™(@µù÷}?ý]À?u¶»?ïI¡¦¥¾
¿çÐ2ÈTB"¿áZœr€À?ÇàE²^.AGNbllRX J1100.3+4019?ïÿ¤¼kã{?	ûGk³Q?Ðå!M?	ûGkµ?ïÜMZEè?€Úd5 Åñ?qÙRÝ{Œ?€Úd5 Åñ?ï©(4Ž?ƒà"üÄ>?…ºú5òÜÅ?ƒà"üÄ>?ïÿL–i'?—®úm?m2Í¿uÏ?—®ú3FGL J1101.5+4106@eÁŠŸb0@O½ÿôA†À:U€[À;Ð>åE¿ø¾"y@JDâˆõ?üK_¯+¿ésã@pw¿ÀƬ†J N¿Ûï kfg¿»|,êLmAGNbllRX J1101.3+4108?ïüíb+8?:ãC? §?8—4î¦E"?:ãC? Ú?ïӗ»îŠ?"£ùq)ó?v4"·º?"£ùq)ó?ï²r]?!†?'i­"—"?ƒch°7ž|?'i­"—?ïÿ§Çn{5?
 fb)Ø?$a2ô:?
 fb(Ü3FGL J1101.9-6053@r ¿p¿é±}À9rÀ7Õ8[' NÀ9Ò%çñ?ý'¤ö!d@	1‡úŠË @	¢®@D¿?â̤žZs"¿àW6³t ¿è…ÂÖ[¿íUç}¨!rOTHERspp?%5!]§Ÿh?$sw
ð?ïþ¬­ê%†?$sw
ð?&û=¤Í ?DY¸"@E?ïþL%³$?DY¸"@E?yŽ»ÞòÓÓ?wˆÓ£h›º?ïÌâˆBY?wˆÓ£h›»?K͖QwAí?D–o#²æ—?ïùšk¢/?D–o#²æ—3FGL J1103.1+1155@mÐ~KZ@N4_²?À9œ''%àÀ;Àæ"ß(¿÷ÒL%r€P@Eõa™š@#²`dä	vW0y¬¿çàVqH9!¿éFûzgص¿Üê¦+ù-(AGNfsrqTXS 1100+122?ïÿŽã+;?ãÉSð¹‡?G5<ñ6?ãÉSð¹"?ïÑ;XTí?†Þê?wbSüU‰°?†Þê?ï¿oT¸Ðc?{ÑpWW?€$*ÑËç'?{ÑpWU?ïÿûü:Y>Å=*1L?>À›'Äi>Å=*1Aƒ3FGL J1103.5-2329@q×®6	@@‰¿¿ž!À9á¢çrÀ;lelkc%¿ì¼A/±Y»@Èvç'÷?úPúa¤¶?ïõz?ƒš÷¿ãx39W(u¿Ø;âŒÛ"Ù¿¶y‰âJAGNbll1ES 1101-232?ïý–—ìü?6sÆX?d‹?3K@Ÿ`'þ?6sÆX?d"?ïÕÜec.?ærþ-+r?uÍN8i-?ærþ-+m?ïc¬*íZ?‰=N›…´?"Šz¢T½¼?‰=N›…®?ïú \†tµ?O†@g­?E~æ-(~?O†@g®3FGL J1103.9-5357@qöÌÈó#@—Þ_ò.À7ø_ð*ŸçÀ:׀·J"‰?óˆg¢Ñ{³@Ö[uòu@$6ým(¢¿àOéÜÊh;¿âý#6pY¿ã£¨™ÅA¿äfÈ\¶ËjAGNbllPKS 1101-536?ïúßÍ[?Lè"&ö÷»?Gð€Ê'Îc?Lè"&ö÷œ?ïƒêìJ½p?£z…*°6?DíP¤?£z…*°5?î´éÿ¸/?˜™ŽQ?¤±h|ü?˜™ŽQ?ïŒõ…ì?$—X:?ŸaOBˆ?$—X<3FGL J1104.3+0730@nµ‹¿PãG@Lõµ ÝDÀ9'UM9oÀ;­`˜ÇÃ?¡¹‡YQà/@ÖR²o@‹s'ÿÝñ»+5q¿æe ó$¿ã'åcË,¿Ù(•M¸"NAGNbllMG1 J110424+0730?ïþt¥$?0ÀÆæ
ü?(µ®~ý½Ñ?0ÀÆæ
ß?ï«öèÉ1B?—ê²â?…Eͳ¯Å?—ê²â?ï'J'‹/B?‡æ	ñ‰?‹mv4/ž?‡æ	ñ‹?ï¾­ía
Ö?tÚX¿å?€T"§½Jí?tÚX¿å3FGL J1104.4+3812@fzv@c^@PB7¿õMõÀ5®à×E̓À9²‹-Æè¿àµƒíñF@æbu+?üX¥€'œR¿×Dû]õ¿Ýn(#¤¿×ÌæäŒBT¿ÔZ½#AGNBLLMkn 421?ïVŒµ|?ª‡Ž¥Énß?•<ŽiPu?ª‡Ž¥Énß?ïÕV±ÐAd?";ëqÈBm?uT§ßNV?";ëqÈBm?í€ÀOE?§•Æ»£q?³ùûƒ…Ô?§•Æ»£q?ïÿüxîO>à'Ù¹Ó™‹>¿t8ƒ…>à'Ù¹Ó˜á3FGL J1105.2-6113@r(ßÒc¿îðÉ'ÀÀ7å8ÇǪÀ:)óð?âö''ž!á@7Ý¢@v;Ÿ"X¸¿äƒAy$·£¿èbz–ý˜¿ííÃ3é3¿ÖÜßb]áPSRPSRPSR J1105-6107?ßÆþ°8ª?Ñâ8cÉ`b?à€§ã÷¬?Ñâ8cÉ`b?äb<%é?ÓA.!Øx	?×;͇´,á?ÓA.!Øx	?ÞúØ+«~Š?ÃmBàCˆ?à'"ê*@»?ÃmBàCˆ?ë¡s
¨|S?¶wz÷ÞdE?Áz3É^¯?¶wz÷ÞdE3FGL J1105.9+2814@i¢ß"xî@P«à"'À9¾‡«ÚÀ;Á¹žòžî¿Úãå¹þ@¹F–<lî@¼¾@Bo¿ç7âR1Œ¿ã_¾«e¸°¿ç½®J;ô‰¿é—ùUŽIQAGNfsrqMG2 J110606+2812?ïø¹Dw
c?Q? 
Gœ?Mî#ÊuJ?Q? 
G¦?ïÏCg!V?…ô X›`?x|^LoTó?…ô X›`?îÓñN YK?š,½úY?¢ÀëúkN?š,½úY?ïú'ùd?EÐ딒Ã?E»¨oÆ}?EÐ딒Ãm3FGL J1106.4-3643@qˆvŸÏ=À@5‡Fÿ˜ÑóÀ9e‹rXÀ;¡6Ç<j¿òñî»ÚŒ@‹U@¤4þ@V)«0ñ¿äÈé˜+ý¬¿äþÍGñÜ&¿×ä&íÌîþ¿ì1 x½ÎOAGNbcuPMN J1106-3647?ïgý7é7g?—«×ä]fî?"YÙ?—«×ä]fî?ïÏ¥IzÚ?ƒÇé¬:?x-q[B'¬?ƒÇé¬<?ìˆ:§W´?¨µZ¹'Ž?»¿¾*ÅBj?¨µZ¹'?ïøâô'yŒ?OÿOù™–?Lt-ºÐ[?OÿOù™‰3FGL J1107.4-4447@qÃN?þó'@,‰9¡}ãÀ8ÉÔCédÀ;bŠ÷??åÕè K‹@…B(o@¶@ @&¿åݚ?½¿êõ†ÿ'å¿âK>}ý¿ïÿÛ*f8¢AGNfsrqPKS 1104-445?ïÿXšz|Á?›«â|¢~?ì°°gڈ?›«â|¢&?ﻖ,oea?‰‡@@Z+¶?tä&§©?‰‡@@Z+µ?ïA¶Š@Ï?"&ïdáp?œ—É.·åñ?"&ïdáq?ïy*­7á¹?'"èÍvé?ÚªYÈÒ?'"èÍvé3FGL J1107.5+0223@o«àe0@Kv 8ðÀ:(¯K²†À;´p'I¿Ë";ϗŠÿ@tRY«î@¿à߃ü¬ìæ¿åá̧ý¤¿çN±Š"±¿¼
-Ux­fAGNbllNVSS J110735+022225?ï垼{¥ò?t%Y
?jaC"Z
'?t%Y
?領F܆?Ú¸zã?†RîzˆÞd?Ú¸zã?îÅagÖ>ÿ?žb͐	?£©é'œ?žb͐	
?ïÙª!z?o‡É`8ª?s*ñýoBÖ?o‡É`8§3FGL J1107.8+1502@mIÎ ‰ãC@Oˆa .QÀ9®JGKîìÀ;«å3Ëßg?ч–u*'@"þ¾·`T?ÿÙGŸP覿á
/±|¿àVY/"Þ¿Ó‡Twüeí¿äþw}¶^AGNbllRX J1107.7+1502?ïÄh³I,S?…z'ç³T¯?}˦[i×[?…z'ç³T­?ï0yŒ,2·?¡TâýâOá?™ðÎzy©?¡TâýâOà?ïj~^¨ß?ŠÖ¾§(¤?'½p4*ä1?ŠÖ¾§(¤?îX™]ÒY?
Òt-´?ª~æj"Ú[?
Òt-´3FGL J1109.4+2411@jÏu@‰]@P·þ¿ù³À:\ø³¥À;ՎñŸêì¿ëœMÑD*Ò@
œ¯ê"Ý?þ0§á6¼?ÏQ–íå¿æŒâaÖ׿ßÐïì·xÓ¿ ­Ð¬*AGNbll1ES 1106+244?ïþ"ÛÄdæ?(#É\]y@?&²C¹±ªK?(#É\]xâ?ïÝ`	ó­¯?€'B5""t?qOû)(?€'B5""s?ïd^bä¹?"±/DÄý?Œ¦ègFÑÒ?"±/DÄø?ïýb'Û ?8/"õ/«?7<ëq"ûA?8/"õ/ªõ3FGL J1109.4-4815@qß%¿­)™@&r¬azŠÀ9¥—­[îÀ;z÷Zï:?æbÈ
í Ï@_Kä/@ôÖ ˆ‹ª¿ç8äl?ˆ¿æuºIðí¿ég#™Ñ烿çÌñZAGNbcuPMN J1109-4815?ïwz
ºí?˜`˜XÓL"?'0¾¨¢5?˜`˜XÓL"?éÓöž˜?ÌûQœš?È°%‡ŸÎ?ÌûQœš?ìiÄßxË?ª¶ã¨qn?¼±Ù9§Î?ª¶ã¨qn?ÞD9òé¹Á?½|J‡
?àÝã‹#?½|J‡3FGL J1109.6+3734@fµ'Ì÷@P>àŸ°À:ٟâˆö´À;íܜM©?ىƒ•þ@
ËØ:&—?ú^Çá?â
¶?äê?ïø̜§h¿ÌŽCE鳿̸@	¹ŒAGNbllNVSS J110938+373609?ïçâÕ^]?qNÚøIÿ?ho*¡£‹?qNÚøIÿ?ïp€¤€}«?¡Vót,?'ïëoðJ€?¡Vót,?îöbüÃc?"2ÅèZ%È? ™Ð3ÉÏ
?"2ÅèZ%Æ?í90?©ç)dÛûÕ?°ƒ»N6p?©ç)dÛûÕ3FGL J1110.0+7134@`µJ`"@E°…ߨq¤À:P­'tâ*À<î
46h?â¸D{"@ƒ`ݐio@>îÿ|¢h¿ã5~VƒV¿ä¿ß"ƒ7á¿Ñú,›-\¿äDŠã76AGNbllRX J1110.5+7133?ïël…˜x?m—kÚþàØ?dp"zg†?m—kÚþàÕ?»nÚ?ªZÚ'Þ2ª?§>VôIJ?ªZÚ'Þ2ª?ï3e`&+?–3¾c½?™"Sû/Ú§?–3¾c½?íPƒÐ]	–?¥€~3ê?µ{á}³M?¥€~3ê3FGL J1110.4-1835@q6_Ø­¬@CȾâ(À9Pc¥ÁÆ	À;uéÀ"š_?å'ÎÕÌ@x^áaÚ@)? ~æ?žÞ¤Kàdj¿ãzuNX¿Þ¦¤*Ru)¿Þ÷Aö¢>AGNbllCRATES J1110-1835?ïÒ>ªdó›?ug‡×•YÉ?vàªÍ†2º?ug‡×•YÉ?ï:_¾
Ö­?š…2˜¾ß?˜´>¥*T?š…2˜¾ß?îÞž×î¿?— §lYãÉ?¢ö#?— §lYãÉ?ìüô±k	€?¡¸b˜a?¸Zt§³ÿ?¡¸b˜a3FGL J1111.9-6058@r2iŸ¡—¿Ù<ޟªw/À7æ>)0zòÀ9ôúWI'ñ?ú…aêhi@0{âN"8?ü}¶¬¤ä&?ïÿ‡¨3¿áÈ%Qâ傿å<"Qw°ª¿êý~ñL³ãPSRPSRPSR J1112-6103?¸É6dóÑ?ÆHt¯Ä?ìæßy3a…?ÆHt¯Ä?¤"%80M?³[ÌéŠ?î½ß
¬|ü?³[ÌéŠ?ÆLµØ'Õ?¶)ºÏ· J?ê,҉ßK?¶)ºÏ· K?՝¹Ç"#?µRUiѹ´?ê›Ø'Ž7?µRUiѹ´3FGL J1111.9-6038@r0Žàm"¿¶nŸËùÀ74éœlÀ:Í<^U @Veòùg@¿lÛËmQ?û'ýXZßõ¿àÍD@÷–û¿àŸ|Ò¹uØ¿ã@Pó7š¡¿èŒZ{v™OTHERspp?u_4ès?|€V`úÙ?ïÕïÍA–/?|€V`úÙ?48ØL?ì?LÜDÛ—?ïýxäöx?LÜDÛ—?ƙV[??²]@Á6âû?êYªi<1?²]@Á6âú?rÆá¡ò»/?eèŒó"%¬?ïÚr<¼‰?eèŒó"%¬3FGL J1112.4+3449@gZã`'@Pàg@™ÅÀ8ðùÏ5]À;­Ôèë?ôÉ5M¿¦t@v˜¼¤áv@Á»=iè¿Ü €±žÒ¿æ·¶Õê'À¿éÇRºb¿ç6–ŒkU0AGNfsrqTXS 1109+350?ïùqîÒԅ?MJFš59?J8D´­í+?MJFš59?ït!$÷?›£Ñž"uÈ?'}Ý;Û`ú?›£Ñž"uÈ?î
Än£+?¡ß9éŒ?¯#¹Î}I?¡ß9é?ìc´5‹½?«Ù/å÷>ï?¼â_S¢?«Ù/å÷>ð3FGL J1112.6+1749@l¿VÀÖõE@PZßÎ1QÀ:×ï¤h)µÀ;Òÿ¬óéq?âº_ð*Ÿç@ó×QÑ?÷x‰ ¥'õ¿í-?ö‡~¿àåñ!ö¿Í`E|®HË¿³"‹RYBAGNbll1RXS J111224.2+175131?ïæ¬ÍřÜ?oƒ|Fêƒ?iS2:f#í?oƒ|Fê€?ï†Zjh"7?¡ï'泶´?ŽieeÛ2D?¡ï'泶´?îúh±yþ?•dDäƒÕ5? Ytèo€$?•dDäƒÕ5?î×Qù"ŽN?¡=ßGØv?¢ŠàfÇ?¡=ßGØv3FGL J1117.0+2014@l2؈v\@P×°`À8œnØû¯8À;"pdìêÀi·|¯Þ@=oxˆÒÍ?ýÝÎg¿Ø£f^P9Ì¿Ý,éo<EM¿Û•7	V•ä¿ÚžoP^«÷AGNbllRBS 0958?ïÿm•pQ¹?ìH°üLJ?MQõÈîR?ìH°üM??ïڀߙϭ?"`oµß ‰?r¿3)Ý?"`oµß ‰?ïÃ:ªŠ0?'™þQ7?~büªºç•?'™þQ<?ïÿøÏ8›É>ݐ‰Å›>ÌÐßU€>ݐ‰Å 43FGL J1117.3+2546@jgžÿŸ‡ð@Q:þßÙïËÀ:']æe$GÀ<
µùK°Ø¿ä…–À l@
]zž,@,Ù¿úVs¿é&•‹Bõ¿ÃÑ9æM¿å(©òçz¿êaÃ$#îAGNbllRX J1117.6+2548?ë¤Î—
KÏ?ÀP—‡Š??ÁlÅ£ÖÐÁ?ÀP—‡Š??î¢K\"GÏ?µWr«"1?¥ÛJ6˃?µWr«"0?ê‡çåîŠ?±u°wZÁá?Åà`kèEÙ?±u°wZÁá?ïÝEg÷?›øg
•?ŸdWS!9?›øg
•3FGL J1117.7-4632@qéî@…+N@*¯a	/TÀ9…oîMPÀ;tÿ^Ë?õ{ât(ñ¼@ÁQ&
ZÜ@qA%iǿѱg
üx¿ë2ÉlCÉ¿è…î)qq¿ÖÏ,;OêØAGNfsrqPKS 1116-46?îòؑý@?¨hVHÝ? ÒvîÐ,?¨hVHÝ?ïO[œ9?® 
8i?œŸÖŒxÈ?® 
8i?ëA{¢=o²?ª·…+UñÄ?Âúw
A9?ª·…+UñÂ?å¢Màä?ðd>'?ÕÅæ»d>6?ðd>'3FGL J1117.9+5355@b¦²_c<æ@MÑ?ùSÀ9ŠKn"['À;µ?Cä?èY²òÂ;
@¾Æ/ú™?þâà?Ee:¿ãTö0À´ˆ¿Û¹Ò;C}¿Ü|¸¦²Ì¿ÜdŽ="¨ÕAGNbllNVSS J111757+535553?ï×4šY5…?uÏ`9~ÍL?te²Óe=N?uÏ`9~ÍI?îÈÅFH|?©;§ÍTv?£s«›x>!?©;§ÍTv?ïïYåÃz?"~ûð›Nd?ŸÃGœ?"~ûð›Nb?ëœL*9Œ?¬–=»n»??ÁŽÏãWÒ?¬–=»n»?3FGL J1118.2-0411@p{1\1@I·ª RÀ93_?*¸:À;ˆüàÎð?ò_9ßÞè@™+û[€"@…è j¿ã1Ró9j|¿é–žN¸ä¿è_x՘'!¿ïølD"@AGNagnPMN J1118-0413?ïünþó"(?=ªªÄ"fÇ?<ˆcÞ»r?=ªªÄ"fÞ?ï¨Rô÷?[3Œó}?…ë{üÂw?[3Œó|?î×åŽõ_X?˜Aiec'ó?¢§ª
‰?˜Aiec'ö?ïçÕaæòš?b,"aFý?h*ž
fÝ?b,"aFþ3FGL J1119.1-6127@rBTߋr¿áVnßå6À70ˆzdØÀ:I=tՔò?ꦥ3‰Lù@ŽzóXh@ßÆ´{G¿Ý"û10›÷¿å-æ‹Ý¿åÆFª0¿è–Ý
Bà6PSRPSRPSR J1119-6127?äsÆv?Џ}^òZ·?×sãÅ?Џ}^òZ·?±§í9uš?Á"î÷²¾E?íË¢XÑN?Á"î÷²¾E?áQë]&f<?Á8rj׸?Ý\)E³3†?Á8rj׸?Õã#T?À¤]]ï?å~ŽyîwV?À¤]]ï3FGL J1119.7-3046@qŠA [À@<J€VÒuÀ:¼*JVegÀ;ÔËÔI¿×)»9t@"e²â?ü?ø¡, qúï?ÕQ{ˆ6šÇ¿è3Ñ\î1e?é
bh™¶9¿Ï€Œí¹¬_AGNbll1RXS J111941.0-304652?ïü"
uT?>Î>Awg?>ï¬Ug§?>Î>Awc?ï×EAï?€s¹'ˆB?tqÝ_9?€s¹'ˆC?ï"K‰ÊŸe?…ÇôL^½ä?ŠíX'3?…ÇôL^½à?ïþê;>y/?6̪×ÙI9?!\Lm*[?6̪×ÙI93FGL J1120.8+4212@dúë__(@PŠ¿Ý/ñÀ8Ç¿ÝÑÀ;øãú?ÖNL¿ g@ÿyZ3þ	?ùܒÉ仿â_qü¶cC¿Ôô¬'Ýóï¿ÎÃÕÍ|u¿ÇG¶Üå7—AGNbllRBS 0970?ï{i¥?ÿ¬JEÝZ?'ÞŽK_¥?ÿ¬JEÝ[?ïtJOìË?—èU©³^?'|Ö¶fµ?—èU©³^?îŠØŠàwD?œ°!«Jyª?§RwQø‹Ã?œ°!«Jy¬?í¿W—ç8Ð?¨¨Ÿ­*?²C@Æ9ƒ?¨¨Ÿ­*3FGL J1121.4-0554@p£Â # –@I9PßìdBÀ8H]®îÀ;NO~ÃT~?ñ¶O)Þ˨@ÌápGæŸ@î"ßu›ã¿à±`²iÁ‡¿æ'þ'o¿ãÀ¥«ºrF¿ìd{йtAGNfsrqPKS 1118-05?ïØMàZˆ?qu¯k-¥º?sÙ}Ò¼^?qu¯k-¥¹?ï¾)Ún?Žúr¸Ð¡?€u‰$yj?Žúr¸Ð¡?ínFlv'? Ô<Zó¢Z?´ÌœKwm? Ô<Zó¢\?ïþR·µú?)yQ?*Ԅ¦ðgç?)yQ~â3FGL J1123.2-6415@rX'ßüTzÀA¯ó£À8\š1o
ÕÀ:áN_¤?ø&»˜Çâ'@g?A‰b?@å¿ÚËè÷¿ä[[¸ã`ã¿êŒ#0J_¿ëd—iò¸¿áHê¥êzAGNbcuAT20G J112319-641735?ïó¥ÒVûe?f¾Ê˜O‰n?X´[R	65?f¾Ê˜O‰m?í"6éE%?Â)¿¨µ?³gVHµÖÌ?Â)¿¨µ?í˜Íÿ'?¤uX¨î!c?³?ùu?¤uX¨î!b?îÇÉ\¸Pô?š.?±'4Q?£ƒj4zð¹?š.?±'4Q3FGL J1123.6+7231@`xÀ Ç@EˆßÊÖSÀ; ýŠúaÀ<*%@+i:?ñ_ &P¡®@	†ÁEA?ù~sÝ@
¿ì'‹'nŒƒ¿â ×@n¿á^ȓy'?Á.å»Ü´AGNbllRX J1123.8+7230?î›"í³ Ý?±…FѶg?¦F±$Åò-?±…FѶg?î_ŒÐ?¼é>F‹Þ?®JG2þ•?¼é>F‹Þ?éiR!?²cNÚ­?Ê[ò·{£é?²cNÚ®?æĬdë*^?ÈaT¹Ý'?Òv§6)«D?ÈaT¹Ý'3FGL J1123.9-3653@qÁY_í¦a@6Â<à[À9
´br»ßÀ;Œ[™ƒÊ$?ÿ>åCJü@X°få'A?úšÚ\ˆ–¿Ñ ˜Å'οÜëYοáZŒÿ_úš¿íZå˜ÞPSRPSRPSR J1124-3653?IDXQÖ?=˜jzÁVO?ïù®éë¼ú?=˜jzÁVO?oáތùº?}e'ˆ´9Ú?ïà÷!s?}e'ˆ´9Ú?‰Ešù®"¼?'ª…Œ]?ïšé"E¬?'ª…ŒZ?gæ4ˆ`Í?UZBøgi?ïèËwŸ3?UZBøgi3FGL J1124.1+2337@kDÛ@-¹@Q€%ߙXÀ9ºJ«õ¼°À;ÛjÕ`ð¿ö9ühEä'@W©¯¼EÁ@¬=?üoR¿å(þ§Ê¿è‰.+PU¿ßžo¸…Ô&¿ê®ûC€AGNfsrqOM 235?ïýƒ-¤3ü?4hX}3ê?3æ'Þ`é?4hX}3Ý?ïÉlE$W?‡¯!MÂu¯?{IÝmÀUÈ?‡¯!MÂu¯?7OšA?‰QO0E2m?‹Pr,oŠ?‰QO0E2l?ïúé'‡Óu?K$½:	?D[aà²*%?K$½:	3FGL J1124.5-5915@r@@ Ç?ü5:ßÏÞÐÀ7ƒ¸µ¾"NÀ:|{üР—@&,§¨Ðï@¨Ù>Ú[@ƚŽ½¿ßل ä¶¿ã}á·aøæ¿é[J÷š¿ëet®/PSRPSRPSR J1124-5916?Bñw³L?G,¢)ñgt?ïû}â/?G,¢)ñgt?.÷éC?G¼h'ñÕ?ïþÏÀn?G¼h'ñÕ?¡Š×@ˆú?˜¡ë"84û?îæ'R‹÷p?˜¡ë"84ü?;|¡.Ñ&'?3ÅXkd¨?ïükÚ%Û?3ÅXkd§3FGL J1124.9+4932@c4ú D®†@O /µÐÀ:dpA±{8À;탠Uu¿Õ.Bç
ô=@pG´Iž/?üل`wd¿êÛÆwž5¿Ü‹æ¨b'¿Ó›'Uy¿ÃžN¬'ÍAGNbllGB6 J1124+4933?ïü±™¿'?IÍ2ØÖ9?:s2k|?IÍ2ØÖ$?ïÁšSž¢/?‰"Ž J‹]?2Ö0®è\?‰"Ž J‹]?ïn:¤jÞB?'šáfX|?'8«r¤7À?'šáfX}?ïûu/"ýy?>҉ÀPué?B+A°
"?>҉ÀPuÆ3FGL J1125.0-2101@qT%à.©a@BÀy`>.9À9øŠ(Ž"À;"ýs]Å®¿'½É;²Y@
÷áíEh??üŒ»à@r¿ï`ó˜ÇZ?é<Õõ"@¿â8Îò'5Š¿ÆÿxñƒeAGNbcuPMN J1125-2100?ï÷Ù¯+ªò?MeŽ'÷,?PL¡¨ªJ?MeŽ'÷6?ï Ìÿüu?'Ÿíxb@6?‡ÌÀ⸏?'Ÿíxb@6?ï ËžjÓ¢?"+ààªÿ?‡ÍeK¢?"+àà«?ï'Îû¬¥ô?†ÈA¶<
?‹ŒAփb?†ÈA¶<
3FGL J1125.3-5824@r=y?ò^W@Î0àµÃÀ8ôËá©ÔÀ:§TÚLè?ñ¬·xÒ¤¨@
ÆG²œ@‡_ZX'?í´…hñ¿æ[›l-¿ßìÅÇ¿íV" ÞÇÌPSRPSRPSR J1125-5825?¡C5ØÀ‡?¯ e"Ä[?îëÌ¢sþç?¯ e"Ä[?Éíy"aª£?Ïoæ'@´k?鄡žç•W?Ïoæ'@´l?ËØ ki?´Ûx%xP†?é	û8÷å&?´Ûx%xP†?ÐzŸ~ö½?¼k^(OP%?ç°v@"¡?¼k^(OP%3FGL J1125.5-3558@qÀ» 1ί@7»'ÿùJÀ9LPtTfÀ;ZHþv"?Óɯ
@§²@h"qM?þ"tÿ±Pš¿Â¦¹r|õ¿Ú·µìêD¿ÚÈoT†¿ÙZÝsZAGNbllPMN J1125-3556?ïýF¦ŸTÐ?7Nò‡(§D?5ÊËY‡à?7Nò‡(§:?ïÓ(‰"É?~GÊ—?vkð;6Ú?~GÊ•?ïÂ;[ 8I?}M«
Uü?~âR/ãÛp?}M«
Uû?ïޟTíC#?`Ú`í%‹?p°U‰^o&?`Ú`í%Œ3FGL J1125.6-6012@rG[€#¦Î?ìû8ÀcïÀ9*]ÔÏÀ:²Qaòc_?î%%‹ç@ö%ÍD@ýÔ¿_{ç¿Ãîü'Ob¿æ̑'§†9¿èT–cjnÅ¿ä25w08,PSRpsrPSR J1125-6014?à)`#0©?Ñی@qº?ß­?¹ž­õ?Ñی@qº?ßáq7?ÔSœ0½?àpÇuùå?ÔSœ0½?â:·íÏH?Àw[íä}?ۋæ$ap?Àw[íä}?â&Šv'?ÀyÎÎ0$?Û²ëßÄÝ?ÀyÎÎ0$3FGL J1125.8-0745@pÒäÿÉy[@H·&_æ¥À:oæÃ%À;ÎCG}m?'É£a>jf@ˆÚY¨=?ÿB*Z~&¿ç­¨,·÷†?ÒwF™¨™M¿äÉns{"¿ÙªaµEAGNbll1RXS J112551.6-074219?ïá'"è?qkQOŠó??nnÝáõ?qkQOŠó@?ïQû­éô?›øõa,´è?•ÀŸŠBÁ€?›øõa,´ç?ï)	[֕å?"uè?|º^?šÞԅ-Ck?"uè?|º_?ïBÜsTÝ?iÔ™éf?—¤qŒUdL?iÔ™ég3FGL J1125.9+2007@l`xÜ@QO?Ï"èÀ:k™èsòÀ;÷úŠu9h?Þ[g/ö#@'ð=?Q@}?pÙ1¿yt]þkˆî¿ç	Ž8f¿Ûš+5Ÿy¿ïÿÎÍ&ÌAGNfsrq4C +20.25?ïÑúò"›Q?ˆ
ì6ó/?w†µ²WŸ?ˆ
ì6ó/?í¿Õߊö?³úºkëÑ?²Q¯PQ?³úºkëÑ?ì:i¯Tµ?«¥&òº.?¾,·:…ZG?«¥&òº.?ë&ÐÀ–º?³už¸{p?Ãg¤¼ý¥?³už¸{p3FGL J1126.7-3834@qÔ_'`@5aTÿ5Õ¥À9üËE%¤À;µïXz?Ü{Fþþ3ˆ@ým"V_@)_ÊÀÙ¿¨Wx6ó\.¿ãü狃Æ
¿é¢<a@ró¿ÎìAÁ/N'AGNbcuPKS 1124-382?ëÖéÛÈG–?ê·»°Á?À¤XÞá©?ê·»°Á?…E·%?œ;X›TµG?ŽÜ®'6þ?œ;X›TµG?ë'?³ÃcQ?´ÿÀlðÇÔ?Á»0òr»?´ÿÀlðÇÖ?í̍éxp×?§mÍd÷X?±›´<yF?§mÍd÷Y3FGL J1127.0-1857@qK…ߨq¤@Cʉ€Fâ=À7R_IÀ:æ3hXÔ?øbýPMJa@ð"gXSÔ@/8Ç¢¿àD¹¦h¿ä@W¡&«»¿åC¬':׿æ¥N…ÁlêAGNfsrqPKS 1124-186?ïöUê?WfyñäiS?SËáT+äà?Wfyñäib?ïĂºHd÷?ˆ_|ä?}¾¢Û̈́B?ˆ_|ä?ï
¯#3V?•':Mwß?žJœÙ•K?•':Mwß?ïýÞX§ë•?4ՇŽHø?1
:À£[¨?4ՇŽI3FGL J1127.8+3618@f‹-ÿ'+¿@Qƒw`MÉÀ97¢ô§À;¢1¿•¬¥?å,>>v±@"¡Ì@Ë;\_¿Ùúö~ªˆˆ¿ç+Q í²¿åœšQÇÀ@¿ã3÷ã?Ä«AGNfsrqMG2 J112758+3620?ïü´	4UÑ?Aÿ˜|OÕ?:_¶]Q|?Aÿ˜|OÀ?ïҖúî;t?"¨p)‰3·?v´'ˆâE­?"¨p)‰3¸?îÕ؊PŠ?šrŠU,[?¢¢wZød?šrŠU,Z?ïéºå…?_Çlaט?fñEozh?_Çlaס3FGL J1128.0+5921@a§É`0Â@@K[€"ØÀ:hJÆͯKÀ;úÚa
¿é†ƒÛÓa"@
Õ´¿%D@¿¼w¯d¿æÜkûõ.¿æóý¤lA®¿ìzmôWß¿ïÿK'$°AGNfsrqTXS 1125+596?ïø¨oŽ3?U5Žÿ¸?M^C‰Ç7?U5Žÿ·?íˆï¿÷j?½vw‹W?³¸'¸D»?½vw‹W?îS"È&]?Ÿ-n¦µà?®:dz}š&?Ÿ-n¦µá?Ô.Ô?¤´ú»
5?¦×r¸
É?¤´ú»
53FGL J1129.0+3705@f>A [À@Q~³Œ¼À:Rîº]À;ÁXù–Ys?Ö!¥Z@8É˳@¨Yÿа1¿æ^µÀ@ÍP¿ãp«ëº¿Ü(•kÈ·%¿åÌÔkÉôùAGNbllMG2 J112910+3702?ïÿkUç8Ž?·š­Tƒ?•Cî@¦?·š­Ul?ï¾Öç‹6?Šò3¼ ?€JxÆ2°?Šò3¼?ïÓµR,9'?y궢5®?v%Véã?2?y궢5³?ïÇ*÷e?s]ûøÉ_²?|wê¿NE?s]ûøÉ_°3FGL J1129.4-4215@qñÂà°«@2nÀ§û\À:ŠÉòý¹À;¿IÍ©kŸ?ޞÏà
Øl@U¸™9@ݵ_Ƚt¿ê<âcâÓt¿ÖAéV<Äú¿æ/–àÏ­¿ïÿìã~Ñ(AGNbcuSUMSS J113006-421441?ì·Iםy?¾µUY¦ñ,?¿jE±C9?¾µUY¦ñ,?ìsº"Þá(?¹"­Ùƒæ_?¼b+ÙöÃ?¹"­Ùƒæ_?è䅾9w[?µ+òFÓAå?Ìmé"?µ+òFÓAå?è©vô4?´À÷˜ó°?ω[Ž$/3?´À÷˜ó°3FGL J1129.9-1446@q3nÀrKw@EÕñŸêìsÀ8¤˜ÒÊ<ÐÀ;•¯,¨Õw?èãà:5@õ`ªåœR@Kà˜†Ÿ¿è.&Ãۃì¿èTB齿ìUÂõ]¨¿ïÿÆւqúAGNfsrqPKS 1127-14?ïþ•uh?2PIïèåe?.¨®™‰ ?2PIïèå7?ï­-xÙ±?/ë趹?"´¡ø	"Þ?/ë趹?ïlÕk(Ž?*…2B˜?'eRúî^?*…2B?ïËŧ"ž?söü=el"?z,n°ñc?söü=el3FGL J1131.1+5810@a¹/ßÁœ@Köõƒ¥À9üÅ0÷ÑÀ<¯k'ö¿Ù xA@@+­,ôU@EP¿`'³¿æÏÇ~f¿èkçÀÕ.¿ÎÅýtNJU¿çÎ^G^
AGNbll1RXS J113117.8+580911?ïú,°@¹)?P´àîË2?GM>ýYÝ?P´àîË-?ï=ë¬jÍ^?¡oª€ê«â?˜BŠr¦T*?¡oª€ê«ã?ïf~[ªS"?'K6d.ï¸?"04Šµ›¼?'K6d.ï»?ï¾v\)ò?zòÀŸòY?€{âhõƒs?zòÀŸòT3FGL J1131.4+3819@eÄ_Js@Qv‹`òËÀ9Õô†O9úÀ;?)
»E?âð—	qmÖ@'þ'…@"@ "€¿è¦qYg-¿ê¬Ü-Ë¿á¢Ú- ¿ïÿÞ\
¿SAGNfsrqB2 1128+38?ïû} {³?H5ÌÊ'µø?B~3Š°?H5ÌÊ'µñ?î)p¡bD@?²àÄû(é?­hõéÛ»÷?²àÄû(é?îÑúb¯?˜M"häµ?¢àYÓÕP?˜M"hä³?èYBámR?¹JÜl5,?ΚôzJµÌ?¹JÜl5,3FGL J1131.9-0503@pÒ: WŽ\@JC* dúVÀ9‡;±†ö)À;ž ùt̿햼CxÕ@'
L46@D)ÀmÃÓ¿æ
E")Š_¿ë/gzý;¿ë
r.¤?¶.w•@wAGNbcuPKS 1128-047?ïüñÉ»)ù?<ý¶oV«¥?8q²&°3-?<ý¶oV«¹?ᅵI
J?`‰3av?€í½m\g?`‰3au?ïH½£šý?ŽÄ Ìâc?–þKŒ Y?ŽÄ Ìâf?ïý6I"ϱ?6ƒíÂe?6M¶é'o?6ƒíÂg3FGL J1132.7+0034@pƒõ_þmY@L´Ò_³Ä¾À8x
è³³À;9]¯Þ}?ãÛÏbíû@Æô÷ŽAw@™ _Æå¿Ýߨ¢J˜¿ã	¨ß'¿áÛ£'¬§¿ÝF‹(	AGNbllPKS B1130+008?ïûj‡pÓ?CÓ¦{'ï??BUâ<³‹ñ?CÓ¦{'ïC?ïGçãÚ?ŸäVh´²?—"¼V?ŸäVh´²?ïUƒœm1?G†öˆ¹?•OŒrYß?G†öˆ¹?ícRè?¦Ç_××Mñ?·Sål¹?¦Ç_××Mñ3FGL J1132.8+1015@opÛ ¸l@P=@GDÀ:gÍÀ;È©lut ¿÷EJ!ŒAÂ@
¶ža@ÃÉàhÚ¿èh ¼IX¿é…®w™‹ú¿éˆíñ¤ac¿ÃàJK0]žAGNfsrq4C +10.33?ïÿ½þÈËß?©ïjOɞ?€MÍË?©ïjOÊØ?ï×*´Ïä?"eó8Ôv÷?tj¥÷?"eó8Ôv÷?ï½N7ºy? ÎܽL‡?€¬r<a? ÎܽLŠ?ïÿÎ2®Î‰>ùd‰pŒl>ø樘»äT>ùd‰pˆ3FGL J1135.2-6054@r\åà.©a?ã@?éØÀ7ÅÒtwÀ:°½L&I@‰uҕ
Ä@²,ðÎߢ@ÆÄuw¿ÝxdVRg¿ããõå8Ã/¿åêybru¿ï
$p:PSRPSRLAT PSR J1135-6055?3H;‹¡½a?*Õ	úxù?ïý–øŽ‹Ç?*Õ	úxø?/«`EÐ?Gþ ê,Í?ïþOÙû¢?Gþ ê,Î?ŠÀeZ&ƒ?"¶vØ}ªå?ï•Èþj—f?"¶vØ}ªæ?X¡GZh?Lhu´7tÌ?ïó¯?\rR?Lhu´7tÌ3FGL J1136.1-7411@rœn «†À(+Ö@éÕÀ97oJ:¶µÀ;vReþaš?é"ú|C®'@
{JÍǟ@Þø 7­ì¿äÊ<'zÿäi˜¦ï1j¿çNµýƝ¿ïÿ¦CK.RAGNbcuPKS 1133-739?Ñÿë¾T'?ÊëAFÅÜ!?ç
 Õý·?ÊëAFÅÜ!?­KåîÌ*6?À.…ËWúÓ?î+A¡=]?À.…ËWúÓ?áOîµ|º†?¸!/纹G?Ý`"•Šò?¸!/纹G?¾Îoÿàr?¤sœmÑ?ì&2Àò?¤sœmÑ3FGL J1136.1+7523@`#W`9%»@Diœ@=òÀ:Žã]2À<*rÉK8¿Ô}聴 @ßF&ñ}@h³ UöW¿ì5=Œ«¿Ü£CÑ9Þ¿µ¥úw™®¿ïÿeiûØPSRPSRPSR J1137+7528?ïæ¦##7{?r|U
œØ"?iYÜÜȄ
?r|U
œØ•?ï£2SN?mÍF«ï•?‡3}+,\Ö?mÍF«ï•?í¼é]°â%?¡ýë´v'ø?²µxîÞ?¡ýë´v'÷?ïØÓ. ?lÎe,?s–hï¹9?lÎe,3FGL J1136.4+3405@g‹y¢ƒ@R`×óÀ9ß]ÂSÀ;åðL-Õü¿òƒÐ&žzT@½e{C@ ¢àRG¿çƒvãÈM¿ìWDû»*l¿ßýx=uα¿çQB,Ë:&AGNfsrqMG2 J113627+3408?ïÿÂ+k?	2`²óÃ+>þüjyÊÈr?	2`²óÄ
?ï¿3X†6?Cë}'[?€3)Þr\M?Cë}'Z?ïÂ+
ütÑ?C–†'—?~êzÅ—f?C–†'—?ïû'—Šû?B4}å©&?A·Ý¡Ô}?B4}å©3FGL J1136.6+7009@`|ŸŒ¨@Fӂ PˆÀ8Û°hjÀ;^R_Hdô¿íxGøI)@²ĆW?ý-;·¿ÓFãh3‰ß¿ßºˆÔ©¿Ü";
dS¿Í¥+OO7AGNbllMkn 180?ïÚݶ<I?oé"v¬O?r'$áÛuó?oé"v¬L?Uð¹€?'aòÎÛ?‡êƒÑ ?'aòÎÚ?îöK˜Ã^?"5: 4? ›FsÊÿ?"5: 4?ïòÞÄö5£?aÝØÈ_ä?ZBv"¸í?aÝØÈ_â3FGL J1136.6+6736@`®.oKè@GûrÀü¨À9À®9À;"Í.œ?Òוù&@gғ`DŽ?ûe?õ¹U¿ço@Aä{ë¿Öà0^l¿Ó—öÞx5¿ØF€i"AGNbllRX J1136.5+6737?ïõOÐÀÜ?VÿY*-
‹?UaÒ^~Gv?VÿY*-
‹?ïp֜Ïî•?•ŒÍï¿6[?'å,f-…?•ŒÍï¿6\?ï˜ÌBy•K?"¿s(?‰Ìïaš­B?"¿s+?ïb
cŽ_?"¯vþ(ÍF?"¾SŽ4ô?"¯vþ(ÍE3FGL J1136.6-6826@r'?…Q
À=™àvpÀ9"Í]"ÍÀ;$É3»o¿ÑW R°Ñï@0˜ZT_S@¯nàˆkt¿çRšNÛ±¿ë>5oÎo¿â™þƒÔ
"¿ç4!ßñBAGNbcuPKS 1133-681?ïñv5‰ÎÈ?_W0d2ðZ?]"ìbo?_W0d2ðV?í3pðn¨?Âð	
J™{?¶c|x|ŠÆ?Âð	
J™{?î%U-"ñ?¡;û¥‰<?­ª­-ÓÄõ?¡;û¥‰;?ïEkc'µa?‹­=¶®Qà?—R"ÉT	?‹­=¶®Qâ3FGL J1136.9+2551@j¡Ì Õbž@RS&@©À:e¾BÆN.À;¿þraFl?âeë^¤j@}þraF?úÝ[ d¹é¿ëœn<7''?Â_âfšœW¿ëD"†âÝ°?á|«¨‡@AGNbllRX J1136.8+2551?ï"Ëâ8¹$?Žjxn²˜?ŠÍqÑ·*?Žjxn²˜?ïÅ 9zEô?Š\À,ӄè?}/ãBÝO?Š\À,ӄè?í]S/¼É?«o–Yv?µc–'­?«o–Yv?ï'j†DÜ?ÄÍg"å¿?zå^nÉ?ÄÍg"å¿3FGL J1138.2+4905@bÙ`Ëò²@OðÓ?­"ùÀ:U:ûÀ<Êý¿³àÀYI&‹Ï@1#õ'´Ð@Í̀{æU¿êÿè¿âxnùÝÒ¿ëèé¸ëÄ_¿ïþÒ
ØkAGNbcuGB6 J1138+4858?ï©Ãô[–†?õž…ÛÉ?…é^Ü?õž…ÛÉ?ïÝ{}î›9?'¬Ãç9s?qBA²d ?'¬Ãç9s?íƒkOB­É?¡´?ÆLÉ?³ä¥…ꑯ?¡´?ÆLÊ?ïÿüÿg6q>ÔI('vå>¸ÆLk#<>ÔI('v'´3FGL J1140.4+1529@nM߆ã´@QtUàeuÀ:¤ü4µêÀ;£ÀÌäJÀ
/0ÁƒÃ@	&z?É?ô $ sRˆ¿ïÿè¤Þ`?ï䉗mðH?ÓùÊÁÚ«]?™õ÷­9ù:AGNbllNVSS J114023+152808?ïþøÇ45?" 
½
‰? sŒ¼¯¨1?" 
½
~?ïُþÛÊ?…$å/âk"?s8€'ß?…$å/âkƒ?î»oÒ¿ó?¡RbsºÞ×?¤IÔpÄ?¡RbsºÞÖ?ïÿÿ[`6M>«4
¾2}>""ù6vo>«4
¾1ô$3FGL J1141.2+6805@`'na«@GÙw·À:%¾<çÀ;ò… ¾Q	?ç`jŠ¶Û@°:6?ùÇ:aOÑ$¿ï÷«z9#…?ïþ9tüèZ¿Å2×BÇ{¿Ëå¢oÔîAGNbcu1RXS J114118.3+680433?ïó¼íV~—?^¹ûÝí?X†%SÔj?^¹ûÝ×?ï'û)tmA?"źÄ(J?‹A5¢ä°?"źÄ(J?ï>'œY?ý["¤8¥?˜-Ì|Ÿ4ñ?ý["¤8¦?ï\•ÆF"Q?ŒÙ̏4˜?"mG7/v?ŒÙ̏4˜3FGL J1141.6-1406@qg¡Ո]@Fµ| À9ô¤	_$SÀ;¿WÜ_çÇ¿àǬø@&Fæ™R@gãà¢J¿äþøÖ7|¿ç†?
 Á¿Ö¢uµ'®_¿âêM{³Õ…AGNbcu1RXS J114142.2-140757?ïýùÉH;?0/Z¦&?07qµ¾&`?0/Z¦/?ï<áÄK?–H6®mþ2?|#Çv"?–H6®mþ2?﹀ýk?(PàÔj?ŸÀ¥8ºÅ?(PàÔg?ïÔèâ‡éä?pSÖ§É*Ê?u‹Ž¼
ì?pSÖ§É*Î3FGL J1142.0+1546@n'¨`ܹª@Q"ßÔŽÀ9ßÞèXÀ;´¥hõX¿ÿx9ܾ@2Qç3Ö@^È •¡½¿ß}3£VÂì¿ä€Óð,£L¿äãތ<å¿Ú1מ7
2AGNbllMG1 J114208+1547?ïû¥ÔxßI?DeÈrU?Ah®'á#?DeÈrU?ïÛ¼\Õ==?';Ãη)8?r!ѕaaå?';Ãη)7?îÏ1<à°·?™ÒeMxÌ´?£ì1ôôˆ?™ÒeMx̳?ïÿ fD°Œ?zšÑTð¹?ænÓÜûL?zšÑTò3FGL J1142.9+0120@p¹7ß (@M·ç 5)­À9Ì·áƒ=7À;Õ§uû.à?ö!sЇA}@
«¼±Ì–?÷Y©™èt¿Ù™‹Ð5ë}¿ÎðCgó7¿ÜN×+܎¿êÎd~§[PSRPSRPSR J1142+0119?àÂ(Q
?Ìþ–F{ÌT?ßÎ{¯]åö?Ìþ–F{ÌT?åRq?Ññ¦E¯'?Õù[ÝÝÿ?Ññ¦E¯'?פæ-ÍÇQ?·XwˆÆª$?ä-ŒéW?·XwˆÆª$?Üy…ô«2×?ÁY5Ÿ¸!¼?áÃ=ªf"?ÁY5Ÿ¸!¼3FGL J1143.0+6123@a® ý;*@Jïä ()À9`¸K5ˆxÀ;ºÜ8zšÑ?ìX€ŒNϾ@}ö۔í@+¯ >ŽÜ¿àFc'²°Ó¿Þ¨ÑM˜˜¿Þ	©æ²•Ù¿ç?+õsAGNbll87GB 114026.7+613850?ë03€'?¾ë"vªñ?Ã?§1ÿ·c?¾ë"vªñ?à—êÏt]?Ï»Ÿøl`?ÞÐ*aéG?Ï»Ÿøl`?ëÉLZnÓ?«ïÚ%ãd?ÀÚΖGд?«ïÚ%ãd?Ú§#í^E?·Ý=Dïï?â¬~î	PÞ?·Ý=Dïî3FGL J1145.1+1935@myA HàD@RBî?äžÀ:Š"#8mÀ;õÙ&wc?®ÒDHî×@
ĎH­˜Õ?ÿ¡7€ô7¿í+ÈÐé¼ó?Äé3ÍY\	¿è±Ëi W¤¿ƒõ­…x"AGNrdg3C 264?O"1Ž?—çÞFx«ª?,7sœh?—çÞFx«©?ïh®%Cu>?£Ö1ܒÅ?'ê;W'XH?£Ö1ܒÅ?íÛIhQï
?§iÒ¯Þ7?±%´½p‡—?§iÒ¯Þ7?ï"°/,rû?˜o½
£ïà?›©úq É?˜o½
£ïà3FGL J1145.8+4425@c}ËßÒc@Q[ÖÀÀ:ß­FÈBÀ<B‹•ÊØ¿§j9DZ`ß@"óM¿üZ?ýšRaKÊY?愈bBH¿Õc8ÉöÑ¿ä:kc{O'¿Ê…û¨¾‹ÓAGNfsrqB3 1143+446A?ïØóT­ƒ?zœŸ]?s†Uÿ)>Š?zœŸ]"?ï'ÈæýÛÆ?–v ™K1´?‹Æ@‰³?–v ™K1³?îXÖ8—? â‰¬ˆ0?ªrœ~f‡? â‰¬ˆ0?ï5·—Z?"ð¥®x@?™_‰
¿–?"ð¥®x?3FGL J1146.8+3958@dŸÙÀe¶=@QÝ­À,«ZÀ7ê$gMÀ;[(fP–ñ?î'l ö«Õ@óN¸IÝð@çÀC&›¿âdTÆßV¿å14œPz¿å^›ÎÔ¿ç蔘AÅAGNfsrqS4 1144+40?ïýžB°E£?02ýî5\$?3
ê}Òì?02ýî5[ÿ?ï×IH1?ƒ2¯ŒHÕ?t[[ç1už?ƒ2¯ŒHÒ?îåŸps†¯?–~¥'¦Ï·?¡¦øǕ?–~¥'¦Ïº?ïþÛ;™1Ì?$zÔ0ZÔ?"LFlã@Á?$zÔ0Z¡3FGL J1147.0-3811@rß 'á@6ø;‡}À8¦ìAÝ"À;l©èœ6,?ê4G;9"G@no+¢@îàrñå¿á¨g€þÔB¿ä¦÷»oÉ¿â®
Á"Žd¿æBDý¤Ê¿AGNfsrqPKS 1144-379?ïÿ߃†3?Ëîú×ð?"9µ/?Ëîúؤ?ï·DÔ ?Œï•šðì?'.܊×ÿÓ?Œï•šðì?ï'ÙÏâÍ?‡dXh-"o?‹I¾ÌM?‡dXh-"l?ïEÜ«@'?ˆ|—Vh–j?—D|ê—ï ?ˆ|—Vh–k3FGL J1147.8-0725@qJJ '§@JÇÀ'áÀ8ÊoÖQ°ÍÀ;g9
É<?Üú(t,;Œ@íËA\k¼@‰V  žñ¿ÛÏ|i¿åå»ëpk¿ä®<ì%¿ä(ï¸_,‹AGNfsrqPKS 1145-071?ïþ™ð¯^e?/6jþš"<?&`õ
¤ ?/6jþšƒè?ï½Nª5?°·øý7ü?€¬Uò¹?°·øý7û?ïhFû"}?ŽQèƒFáf?'÷ ^,?ŽQèƒFáa?ïóµQøHc?RO›ÎÝË?X•\o: ?RO›ÎÝÀ3FGL J1149.5+2443@khÌ Õbž@Rø. &{•À:SYäwä=À;êúµ=d¿ù"øzût@RK»jNÓ@ã"@>^Š¿éI \ŽBÆ¿ÔmPëªÞe¿ç%+~ðI¿à±60"›©AGNbllRX J1149.5+2439?ïï	dÑ°¶?aâ,*û—?`ö›.OHI?aâ,*ûœ?ïÉÀn(ÚP?Ž»ÄcÕï:?{Èë'×â?Ž»ÄcÕï;?îæÎßâB[?˜!JYbý'?¡"ÛÚd?˜!JYbý?ïý»3½nF?:ÏNzN?2&bÇz?:ÏNz23FGL J1150.3+2417@k¥Ë èBt@Rþ)¿ìêzÀ8ÛðòFÀ;Q†Xt5\?½×ë4¨Ž@"úõT*z@³&ÿô"¿áظÀrù¿ã•Lo:P¿ÞyLOÂh£¿è•ñÐ"¨ÞAGNbllOM 280?ïëØCÍÇ?gõ˜†üq?d'¼28€@?gõ˜†üs?ï7"¦-&ä?¡~«š9ÿ??™
‹:[#Í?¡~«š9ÿ??î_ò¬qw?¢#¶Ò±?ªޅ8è'?¢#¶Ò°?îCñü')®? ‰ì¤Ê¤?«Àà6íe? ‰ì¤Ê£3FGL J1150.5+4155@cã{¼¾b@QªÍßòCÀ8P,‰ËÆ=À:î"Z•wÌ?èÚÈ¿™U@Ü"¡À…?ü$PôF¹¿Ñ¦àvo?u¿Û©S1¿Ù
ª©ój,¿Ê=.‰«:AGNbllRBS 1040?î"ûî¿m?¦Ž£ÌÞá?¦ÀAô	?¦Ž£ÌÞâ?ï"|¿øÏ?©í'Ñ+!?û°hæ1?©í'Ñ+!?îoý¶½%?iƒÊÒLt?©$"-®¢?iƒÊÒLt?èãåÒ@n®?¸ÂÁy'<c?Ìph¶þEK?¸ÂÁy'<c3FGL J1151.4-1346@q—¢ŸœèÙ@GIZ _†xÀ:(8_ÂÞ7À;¿?']<¿Õ-Âvî°@éi{Ð?ÿ«@àoí¿ÜZ§žó~¿çÁ Hõ½1¿‰s¯,Ü`¿Ýpà~‡½AGNbllPMN J1151-1347?ïÿG»>ˆn?–S"vK?˜.ò"€?–S"v$?ï«0X?c¼ü?…8ÿsø)ã?c¼û?ïµÈ²¾€?(Rƒ^,†?'û"P_€?(Rƒ^,"?ïø¶L´ð}?G¯—cJ—­?M&Í,>µ?G¯—cJ—¯3FGL J1151.4+5858@a(¿;ê'@L>­¿ÁKÀ9iëBÙÏÀ;¥ÒÐçÝ.»™›@PÍåüs®?þ­&žû-]¿æÑØú†€¿ÙíuÝ/y¿àÖ¾ù$™'¿ÊŽ!%–ŠAGNbllTXS 1148+592?ïüqø֜?;¤åsÏ¡q?<p9KÊ?;¤åsÏ¡9?ïÃéY''í?Š<}"ޝ?~Sl6‰_?Š<}"ޞ?ït(†jõ?‹mB˜˜	?'}zï2¡ ?‹mB˜˜?ïúª
›¼?B\n(LÔp?EWÉɑ€?B\n(LÔk3FGL J1152.3-0841@qq_¿ƒ8.@I¶hÌÀ9(ÇôøÀ;"°Švæç¿ÝÆ Ò@""†g¹@Ž=Àâc¿æO&ŠÈ	]¿ær^E"_¿æç$˜`¿ßf¨ÎôL÷AGNfsrqPKS B1149-084?ïþ,˜,3_?4<c€Ê2÷?-6}<ʽ?4<c€Ê2Â?ï¦nÙç®!?b¦Îó-?†dI†wù?b¦Îó,?ﻆ°¿_ý?~3±z•!	?SÐ(Î?~3±z•!?ïë#ÅbŠ•?`²¯˜Ê"g?dÜ:uk&?`²¯˜Ê"e3FGL J1153.4+4932@b0öÿ:Þ"@P=ÿ%¿­À8Aó‡K¹<À;–w§×Iþ?éCVqÚ@†@I~úï@A{P¿ãÅxãŸ)Ú¿å"ZíƒÈï¿ãIŸá‡D¿ìÁA_yAGNFSRQOM 484?ïò™ÞõØt?`+»ËÍ?ZÌBOs?`+»ËÎ?ïÕcL6î?"=žÐ	"Ì?uNYôdˆñ?"=žÐ	"Ì?îcwç'7p? "˾âR?©ÈŒ‰? "˾âR?ïÿù{ª?>Ô¼©¹u>˞W>Ô¼©¾À3FGL J1153.4+4033@d`Ï‰@Rڀ¶–À:wŽF@À;ÙUËäo?ÍòÒ_*w@Ú[Ü®l?üF!_K??ïúGþÿ¿Ò'¯·µ…Ö¿ÒÑ;Ïíq;¿ÚÝx-Z£‡AGNfsrqB3 1151+408?ïå"i3ÎF?y£	–¶?jl–Ì1ºˆ?y£	–º?ïB&¨l?£ÒZd Î?—»=½Êòp?£ÒZd Í?ï
M%"u£?"ڏD^¿=?žV[MqKž?"ڏD^¿7?íæ¢ãüS?§³)Vuû?°Êèàg?§³)Vuû3FGL J1153.7-2555@qðe¶™…@A"Œ_õ3À: öC¾›²À;à ɤ#`¿ÊF#.§@
ˆùyO!@9 4¾N?ìÕa¤h]¿è"ÍñÔ²ä¿Á7æÁj˜û¿ê8חAGNbcuPMN J1153-2553?ïã^OǬ?tà&#k?læ¡°8Tè?tà&#h?©ý|Æ?«e®®#b?‰PՀ ÎS?«e®®#b?íX3tg¥+?¦%Žì£?µ>d\ÂÖª?¦%Žì£?ï¾¢2O<2?yÚrç‹ÄB?€Wsl0ó!?yÚrç‹ÄE3FGL J1154.0-3243@r²gÇ@<œûÿÀ? À91ÃÇkÀ;iEW"&?ï­qpì¸a@I¼ˆ†÷«@lÅßȧú¿Ü‰I±5'æ¿áˆý&~;g¿Ü@Ö²÷¿æ¾üHÕÆAGNbcuPKS 1151-324?찁ˆS‡¹?´K0¯‰'?º{ó½cÂA?´K0¯‰'?ãjwË[' ?É̏:ìi"?Ù+iHÜ¿?É̏:ìi"?êØ"TAé?®^K%øÏY?ğ›v®øY?®^K%øÏZ?ÛEc°þ?³iPO±ê?â]N'€÷?³iPO±ê3FGL J1154.2-0010@qå¿­)™@M¶xßå®EÀ9ÜW?öÀ;r¤Þq9ÿÀ|v4ÐR@¯9"õjÑ?úð ¦=¿åô"½Ö¿ÝÜSH¿Ô÷"}~c'?£ÀÌó&JAGNbll1RXS J115404.9-001008?ïüÁü¾jÝ?Dl½gžè&?9ð©t?Dl½gžè?ïÒ"ÉÛ7?…älœ;!?vî¸dq?…älœ;!?ï•ÿR½:M?ŒF/4">«?Š€+P±l¥?ŒF/4">¯?ïÿÿ–&:Ý>œßÝ:"}>ŠvqHLJ">œßÝ9¹ã3FGL J1154.3+6023@`é¦Þüz:@K¬ºAn_À9‹æYeÌãÀ;Ã^Zÿ*?â,š-±@{ÅËÑ¥$@AÚ?üð+¿Ö\Ù²ìÆ¿èy˜㳑¿ìšý‹ K~¿å$r3µJ`AGNfsrqRX J1154.0+6022?ïùŽî#?Rò2é?KÅÄGs'?Rò2é?ï~ÎËíh?"'œLv)?>&&'S?"'œLv)?íø¦§×5? øt(:ˆõ?°:ÊÁGNZ? øt(:ˆó?ïP]­Â?rf_÷‡4?•ôJMüǍ?rf_÷‡63FGL J1155.4-3417@rEߨq¤@;(Ràw¤|À:Š…=ÂÀ;š®]uüÜ?ÚÃèNÕÈk@gD¡D³¹?õ]ß>>?ï†	‰ÍI¿ä–.ÙÃfƒ?¯zH<ý¿ÂxrÜ°3~AGNbcuNVSS J115520-341718?ïü•X"ä?B5°Çe×À??#U;Øç[?B5°Çe×Ã?ïКX(úm?îÓ¾s?w²Óë'Êr?îÓ¾s?ïIÛC¯—?'|nÜÖ¦?–Ä—Šl÷?'|nÜÖ§?ïÊ<ö.?zæ¤ïýê?záõù"é=?zæ¤ïýå3FGL J1155.9+6136@`Ʀ?šIÃ@K%v¹ÃÀ:Ïÿt¿Å}À;÷û'Ü5ö?áõûÏS@8H‡®4±?úVÿn4¼¿íÕĘ©bB?ïÛ ±•'´?®ÅEÞ M­¿àÐ3xl<AGNbllSDSS J115548.40+613553.8?ïà哊¯³?xƒ^CÜg?oluPN'?xƒ^CÜh?îi#%«>ž?´b£tŽî?©mÍ¥L#?´b£tŽî?ï']ÿv?'âώ3Ùc?›
ô] ^?'âώ3Ùb?íì	lº?«"ÊÞ	S`?°Ÿ´Ÿ
/¸?«"ÊÞ	S_3FGL J1156.7-2250@qìò?î,™@C'.ÿÇËÜÀ:='¡}"À;¢£Ìhú?à`ðúP@
/FB¯}?þ=~`X/l?ï¶z'A&¿äQƒ¯½¿ÙumKv»¿Â£¼y© AGNbcuNVSS J115633-225004?ï÷*R}µq?S'U'ú?Q«[• ¬?S'U'ö?ï¤ú —¡?'M–´kÏ?†ÁWÚ¿P?'M–´kÏ?ïF>³bÜá?m¾Ñ;¼0?—8)"¤có?m¾Ñ;¼/?ï5~\õß?–îðH.!?Ÿ™P4aD?–îðH."3FGL J1158.8+0941@p­ÿ'+¿@Q&^è¬À9•,D+¨ûÀ;˜È¡ÄáFÀ0°ÿç¬L@«=ø9à@R"`R%<¿Ûiís¡Ÿ¿âì3ˆ©Ão¿à©wÍA¿Ò;'§%ãAGNbllGB6 J1158+0937?ïÿ(ÂÃX?÷'$ÒS?ç¿'•"ƒ?÷'$Ò
ô?ïÜ-¿‡?C]fԙŠ?qüé u<_?C]fԙ‰?:!µ¦?‡;ÇžM?‹qw'–›?‡;ÇžI?ïÿòÆY?'>èƒÖº:Ë>ÚsM€á€·>èƒÖº9Ð3FGL J1158.9+0818@p°ñŸŒ¨@PÜäÀ™,À:§ÎçY@À;ð?HkÈ¿¾ç­xɕ`@¶õlÿÜ?ýéeŸA#a¿ê|Aâx…£¿Óûãl˜Ò¿ÅwKu
7¿Ù­/}ñóMAGNbcuRX J1158.8+0819?ïü!Å°e+?WˆüA€é?>ñÒ|Ö¤§?WˆüA€é?ï¡«¥I'+?•§~mÌ7ˆ?‡•­›´î?•§~mÌ7ˆ?ï8ÌÕ!uÙ?—+.òþad?˜æe[ÑDï?—+.òþae?ïµ,B°\?n!ä…"?'½4ïSé?n!ä…"3FGL J1159.2-2141@qòs?Èlì@CÊÍ_™Ã‹À8Û¼¸''íÀ;>£
¶¡è?×Ò8ôŠ£T@Cˆ™A/@â矶ê¿âóâhž¼¿æ¡y™ÁT¿æiùB÷vo¿àôÓ;YÏAGNfsrqPMN J1159-2142?ïýl,)\?2'%+é(æ?4žžµý°?2'%+é(®?ï»ô%£H?‹€uÿS,?ö—:­º?‹€uÿS.?—M5	?"%=¹"é?ˆ[Ú,²½–?"%=¹"é?ïï}qMa?TÏí‹BrP?`'Ž²žb®?TÏí‹Br[3FGL J1159.3-2226@qö`RP/@Cma .QÀ8…ž8dË\À;ÍèU¿O?ñ_ß0§'¬@&æÓE7@ùSŸQí¿å\¯:ëŽY¿äZDiÁ¿äªP!Å;x¿êŽã4îVAGNbcuPKS 1156-221?ïߖîZ ?u­"JJe?p4õˆÒ°?u­"JJf?ï¨1ô÷ˆ?ŽçÈTù?…ùs'Â×?ŽçÈTù?ëßXþBå?«ÕXÙí¯ñ?À'œ÷äk?«ÕXÙí¯ó?ïNj²'[V?"î>Ÿ×4Ñ?–2©­´•f?"î>Ÿ×4Ò3FGL J1159.5+2914@hî?àH@S—úÀ%À75#Â|ç²À:ؽØ=CW?÷¿·e‡n@E|^Jc&@éý¿]ù¿à7Æíî8¿ã"<b3¿äÂBÀ
¿äcåj}wOAGNfsrqTon 599?ïù&Z¾˜w?Q'´^a+?Kf•ž ´?Q'´^a0?ïҙ™UŽ€?…?"U?J?v³3U8À?…?"U?J?ï'€Àï?•ˆ­ i†»?ŸíÞïçâ?•ˆ­ i†½?ïÿÁ~¥òð?/ûÔ1Ø>ÿ@­‡[Š?/ûÔ153FGL J1200.8+1228@pX: WŽ\@QÊ9`~TÀ:ªŠ'¥aÀ;Ò7yê¿Äf!‹Ú­û@GðÂJgØ@üµ?½Z>¿ãɵî¹Ü…¿Úôê-ðÖ¿èäXòµi¯¿Ò €³2ŒAGNbcuGB6 J1200+1230?í"¤[Ċ??½7 Æ*¾?¶êÝ!Û®?½7 Æ*¿?ï]i
}ñ?£öªœÍ4Ä?"RÞ°_A´?£öªœÍ4Ä?íKÐ8?¯¦Óš×Ã?·§qã~5?¯¦Óš×Â?ï,ãÎɸ?"]Vä¤R?šp†&Èú?"]Vä¤R
3FGL J1200.9+2010@n)<ßï¿@@S!ãŸâˆ÷À:»˜¢úÀ;Ô O*à~¿øâZ=8DÀ@;ªv`¯m@1Œ` ÿ"¿æ0o<+ˆ¿ê?äߓ#¿àvºól¯è¿ïÿåÊ/õ¢AGNbcuTXS 1158+204?ïÿ8Ï*Î?$;ߣ÷Õ?xæ¦A?$;ߣ÷³?ﱍÀŒÚ?•~þ©?ƒœþÜÉ»?•~þ¨?ïhZƒñ¾ò?‹ñ§Œ0?'ô¯È!Î?‹ñ§Œ.?ïùtÂNÙ?QÛpJܖD?J,÷îĞÊ?QÛpJܖJ3FGL J1203.1+6029@`­ñ¾ôœõ@KÑm`U«-À9qɕà§À;Ô#ú±¦¿ø4€z¹¯@²:)Çy§@ªþ¢Lœ¿é<*Fê9¿ÞíÆw'¿á»qä'¿ç™Ä»¹ÞAGNbllSBS 1200+608?ïáùÓÐ?qIð¿ž?nó,/øÀ?qIð¿ž~?ï˜j]ج[?'öÄZŸà?‰åh‰Ôé	?'öÄZŸá?îŸfŸ²¤?œrðÞLIg?¦	–¤ÕÅ?œrðÞLIe?ïøáÕøJÛ?R½Uƒ˜Ù}?Lx¨Ԕ–?R½Uƒ˜Ù{3FGL J1203.2+3847@dààëgÃ@R¥ïß÷KüÀ:k'öjÀ<q/îU¿üÐÚ8M´@fÝ°õ«¾@m!¬ˆŠ¿ãAÿÞЎ¿în-{°?ݯ8gOšr¿ïÿöõ;ŽAGNbllNVSS J120257+385147?ïÚØ."+Ù?˜wu
—ëõ?r"èîê¡?˜wu
—ëö?ンò=·J?"7t¥Ç¦=?€Xƒp'-j?"7t¥Ç¦>?ìüǗÄô?®dzbÖ?¸ÃAßi?®dzbÕ?ïþü c¿?6Çe{Ób? =ùÄ_?6Çe{Ó)3FGL J1203.5-3925@rO@ €@6ƒËßgDÀ:2.¸z/qÀ;—øö ƒ-¿½ÄfÑ	6N@
"Z"
kê?ú7Ó@"TŽ?ì;dÐ9=ä?ïš[ÓæF›¿æÐ3¶Xu?¢¥½‹³ŸLAGNbcuPMN J1203-3926?ÄÙý? 	Í0.Ÿ€?žŒ/çdÀn? 	Í0.Ÿ?︍\Ël]?™¬Qg˜£Ú?Ü¨Í$è·?™¬Qg˜£Ú?í	UD!é2?«Kâ-õþ?·µUÞð¶w?«Kâ-õÿ?ï¡!J[lÎ?ˆ)pð]?‡·­i$Ìy?ˆ)pð^3FGL J1203.9-6243@r˜n «†¿ÖªƒÉbÏÀ7Û5÷2ÑäÀ:*Eå"T?ü$NÂÜ@Sjøœ^p@.jÑ¿á'YŸX…¿åÇVVVu¿çP§'«"¿î'+'uPSRpsrPSR J1203-63?aå8ԑK?`ªc1oáê?ïîÇ+nµ?`ªc1oáê?RñyZ˜<?h\Êò[ ?ïöÀCRµ?h\Êò[ ?½@AŠúlò?®A°"±lw?ìW÷Π²b?®A°"±lw?˜:s—Àp}?‰iWÔÝ?G?ï>,cAü|?‰iWÔÝ?G3FGL J1204.0+1144@pŒy¿ß~€@QÀ»À5ÖÀ9°ÙQÀ;›¢ø½ì_¿ÒR¢v?«@%²A±%?þ	'€J¾¿çVöو'¿ÖßŠ§ä5¿×tæY1¿àœ²ßwªAGNbll1RXS J120413.0+114549?ïþPn÷8$?0ø&Ûy!?*ùŒ}Â?0ø&Ûyl?ïÅî±ß4?Œ U1éµ?}§eñâ?Œ U1é¶?ïÁ®?|§l梗ê?9zv(óì?|§l梗ï?ïëŽ@FÙ?^²£fØ¢¤?dàq¿¹(?^²£fØ¢œ3FGL J1204.3-0708@q­µ?|í'@Jño`
+ÓÀ9böo]†À;BöÕ®?×ýµ(/@ý4XÍ °?ýÇz Z(¿å0–Ý@|¿ÓP–ñH­¿Ô(SÜ '¿âV[À+dïAGNbll1RXS J120417.0-070959?ïáÏht.?kTv¯ð–@?n0—‹÷Ò|?kTv¯ð–<?ï!®1±d¡? ÐO"?›Ê9ÉÓkì? ÐO"?ïJŠÄŽ¤û?}=Ͷ?–®§n+`l?}=͸?îÂ0]Aþ?œ8D©"~?®#Üú+à?œ8D©"~3FGL J1205.4+0412@q5»à~í@P&3`<ÎÀ:.
¦L/ƒÀ;͒ûç2?œ9>ce@ ä}m"@!=ŸÈ²·¿ì/£sžD¿Éë17–«d¿î?`Ɯæ¿ïÿ¹‰¬š0AGNfsrqMG1 J120448+0408?î×o´'ç?¬êÊYï–L?¢‰¾˜?¬êÊYï–K?ì¤"dÀªW?ÁAÈ°8?ºÞìÙú­Q?ÁAÈ°9?éYòõú!t?´‹~åK?ʘ4(z1?´‹~åM?è†Áø>?½ìÞtKªñ?ÍäûüË
?½ìÞtKªñ3FGL J1205.8-2636@r'=ÀTïF@A"ÌÀ7"À9+v2ŒDÀ;v¢À‰Èk?ÒnKa49@}ýîØ»C@S.Ÿz¯¿ä[8€$'¨¿çÒlÁ<‡¿ç'"±UÖ¿à<|+AGNfsrqPKS 1203-26?ïýßè;Dz?4ñ'h†€Ý?1¾%Ü48?4ñ'h†€Ü?ï¨EëD8 ?Ž6¼Qh?…î….ñøW?Ž6¼Qf?ï˘®
áÇ?z‰Óºk2œ?z3¨ú"?z‰Óºk2¥?ïrXab?ƒ,nÇãüú?'¾ôóßS¯?ƒ,nÇãüù3FGL J1207.2-5052@r}©ß—ª¬@&ÉÁ?ÐÐhÀ9É:qÀ;{ö?ŒÝÉ?õÛ£g"Îâ@gwñB"@#à ¼Ž?Üu@å£]¿×K".ùñ&¿åÂHù꽿îaÓZGAPSRpsrPSR J1207-5050?Îv›ý<Í?'š;i¼®?ïyŒK ?'š;i¼®?ÒBÀÑ nu?Ìj&Ëe?æޟ—oÈÆ?Ìj&Ëe?±Î
lÅûÉ?¤i®ƒ&›y?íÆ>²g@‡?¤i®ƒ&›z?Ñ'zöÓK?±EžlŸx?ç6"–Z?±EžlŸx3FGL J1207.6-4537@ro@OÂ@0Õ€ÐtøÀ:4\÷QÜÀ;´²$ªÚ?õ}h%-a@Gý™Heõ@æùÿ_ò¿ç5§«uª¿¯ÃO`Þ¿âyaÅÇÚ¿ïÿõ³¶YAGNbcuPMN J1207-4531?ÄïÌ{x?Őåº3¡?êüDá!û?Őåº3¡?¢1Yhžé?´4¢¢Í˝?îÜêiv?´4¢¢Í˝?ÄëÀ×ñ?°'¢í,4L?êÅ9Ê8"?°'¢í,4K?­Á{܈<Ë?š³ÖD½ér?î#èB7|4?š³ÖD½ér3FGL J1207.6-2232@r¸_.Q@C›ãø¶À9´ýµ¢äœÀ;Œ27Š±¿ád"†Ò@ñ3¼Æ@™@ ¦n¿â¦-QØöã¿éYA}h©¿éÜ ï'¯`¿ÛÉÀ¤õAGNbcuNVSS J120738-223250?ïöÒÖwõ?QP;´ï÷ˆ?RZSé,?QP;´ï÷"?ïrQׯ?"	ÅÃáTà?Œ£_«Šõ?"	ÅÃáTà?ïñŠÓ'B?"lԊsfœ?¡Î¥×Ì?"lԊsfœ?ïŬþºÒ?tÈ•Æ3?})€ø¢˜H?tÈ•Æ33FGL J1208.2-7810c@rÊhŸÆÚEÀ.ùûg¿,À:7jÒñ²À; Ôký¿ó˜Õ¿9¼9@1<6½|@*A`y£¿èþv§kF¿ãOL÷¿ØuEWHw¿à©9c'»HAGNbcuPKS 1205-778 ?ïþŠ†Zsü?#µ1F	1?'WšXÀ<Ë?#µ1F	y?ïÔÃuû¬?'ÃpLɤ ?užE)óW?'ÃpLɤ!?ï½x§Fߌ?~4c¡šç?€¡Ö.HU?~4c¡šô?ïûüAÚï±?BxCÿü?@ø"A=ß?BxCÿã3FGL J1208.7+5442@`úMÓØ@N«"ßöu=À8rS±À;ÃÉfæ¾æ?çĝúZ\@{´+k>@X˜ÀUÆ¿äúÛùî÷x¿æá^‡IàÊ¿ç^Çζ0ÿ¿ïÿâóÍ3AGNfsrqTXS 1206+549?ïý¨P
?<fEä‰*?7Z¿åÿ?<fEä‰*?ïËgÃÿÞ\?†Ÿ¬¿l%‰?zLц?†Ÿ¬¿l%ˆ?ïVÑþ¦ŸÅ?Ž¥tÁ{E?•%À+,c?Ž¥tÁ{C?ïö÷XE/?P­©b§°?RùOuŸ??P­©b§ª3FGL J1209.1-5224@r†o€Uûµ@#܅_û¾'À9ùS‰XÀ;Œ¿Ígý¿öGþ3¢ï@
PëTø@Òc`¢'!¿éË"'È¿ç‰N'«?´¿Ý9iMM¿äø"PŒàNOTHERspp?ïý@×e ¸?76U3c_?5ùDÖú>H?76U3cz?ïՆÚv ?"#‡$kÑ?u<ò'Ä°*?"#‡$kÑ?@ªI?"yõQEr\?‰¯ÕíÕ?"yõQErX?ïüpYpÖ?@z2Û}¸?<}4yO÷…?@z2Û}·3FGL J1209.4+4119@bñàm"@RXfÀ(yœÀ:×YîˆßÀ;ÖEßÞ"¿÷ÁèW´›@SxW)²?ÿ2Àœ'È¿èѸ®Õ"¿á
+¥Rèä¿Ã7DԊB¿ãÏK4åCAGNbllB3 1206+416?ïÿnGÂyˆ?aÀ™?7°Îë–?aÀ™?ï×a™»¤«?ƒh~ëý³?tO3"-«G?ƒh~ëý³?ïÉ
q??}u$÷£Ä?{qùÇ`˜?}u$÷£Ä?ïÿ¡!#Ì
?nå+RlŽ?··ýz?nå+Rlì3FGL J1209.8+1810@oºèÀHZ@S9Y_í¦aÀ9gšA_EáÀ;¬ìµ `]?Ô¾t~
@ÐXAŠŽå@a>ÀZ"¶¿ÝF\ë¾T¿å¡•¹1±Ë¿çmP@Ê¿ãyU­lÆcAGNfsrqMG1 J120953+1809?ïûiËå7`?Kç#cºÎ?BXÐk"ƒ+?Kç#cºå?ïÕ"ù÷¤?ƒäZ´1Ê?unƒ|.-?ƒäZ´1Ë?M1ç?(À@Š?¤T;,ï"?(À@Œ?ïò:Å؄D?UüLævd?[ŠtN÷wš?UüLævb3FGL J1212.2-6251@r§µŸôým¿Ôl(€/mßÀ7ʇJâ|aÀ9Äcôœ¯?ÀùÉ«ÁJŸ@Þao@ç v3¿àU¬9¯N7¿çF& 'Ó.¿é8¡Nè¿ãœ€w_OTHERspp?Õ۲َVÕ?ÐKD‰\G?å&"8Ԗ?ÐKD‰\G?ã2EF:ê?ÕÑQÞþûí?Ù՛usŠ-?ÕÑQÞþûî?Ùíøöe*¼?ºâÚv)‰?ã	"Íj¢?ºâÚv)ˆ?ìp-€ä?º¹Û8Ñ?¿T~"øßs?º¹Û8Ñ3FGL J1212.6+5135@aÍ߆ã´@PM`#UÀ:'tVéñ¡À<ù7Žâ†¿¨n<OÕä@Å´'Œ¶@‡gÿ˜§¿è–'þõ¿¿Ú€]Q®5¿æÍNî-MI¿ã:©xx¦tAGNbll1RXS J121301.8+512942?ï¼ê¿Ö^?‹|`6õ¦ž?€ÅP
xè`?‹|`6õ¦?ïz\'bœ%?›*QP4O?´mÓ¬{h?›*QP4O?î Ø_"`£?žÂÀÞø?¥òzÉõÃ?žÂÀÞõ?ïV7M~â6?>o.SÌ?•9P#¹b?>o.SÍ3FGL J1213.1-2619@rE̟¶M@Aád ;ëÀ:1û9ÈÀ;¢þ‡Yûõ¿ì‹›óÄ{@`•™¯¾õ?þ.Ԟþ2u¿ÞµÁ"I«ñ¿ê¢%ùR«¿Ò‡¥; ?‡ÜèñÜAGNbllRBS 1080?ïÿ<{'_)?ptë¿ñ?p´ÝL?ptë¿Ô?ïÔ¢«AÒ?-™îH$	?u®ª_8:?-™îH$	?Èã"?"ICñÆS?ˆÝüÍÇ?"ICñÆS?ïþó€Lñ?%:ßõ	ª? Çû0ïþä?%:ßõ	ä3FGL J1213.7+1306@pί€Uûµ@R[¢Àh¡À9¦¦J'RÀ;ÁžÊ[…?îâä]&£@r°¹Æµ±@([À6ã¿ãœýd¢Êx¿åݙíÁ'í¿ëÉV~D‡¿ï÷c"ã©AGNfsrq4C +13.46?éèÑYy?ʟý¾¡?È\»¦šø?ʟý¾¡?Ҋ§©ÎË ?Ówiú{?溬+š/?Ówiú{?èèñ7b?´P[ª$æ?Ì]ø;£"x?´P[ª$ç?·]Ȕ"?¤a§ûíÇ?í"FíÍ?¤a§ûíÇ3FGL J1214.0-6236@rªI`0Â@¿ª×'?á
À7Öå•ñnmÀ9Õܨ#$?÷Nu»€Ê@>:\È-?þ¿Ü™žw$¿º}bVa`˜¿ãÜ[ýVØ¿å%±Ím¿ézØC""OTHERspp?gZ|¢ü?pÁ!+4Œ›?ï襃ë]å?pÁ!+4Œ›? 7$˜8²{?±'Ɲz–G?îü¶|tØ?±'Ɲz–H?±ÒŠÐÆC?ªßO1ãMi?íÅ®¼¥ç7?ªßO1ãMh?À|'
#S?°?Æ5‹Â?ëàß}÷+?°?Æ5‹Â3FGL J1215.0+5002@a,ô!-w@Pƒ¾`"‡À9þ1Ýȝ"À;ÔÇýZ3R?Ô¶G5"ØS@RÙþ
·y?þ¶
 r~?ïIJá$É¿çoO ž¿ÁTªYãÔ¯¿åѱ'­AGNbllNVSS J121500+500216?ïýYý?@6äa$
{?7]7÷ˆO?@6äa$
u?ï}â¸FÛ?—|…G'µÙ?C¨÷'Œ|?—|…G'µÚ?\ú7X?…¤ªÜß?ÔèÁr)Ù?…¤ªÜà?ïãp‡»?"'02šF¤?žž'ïœ?"'02šF¥3FGL J1215.1+1658@pW"_ôö@S4z?̞ªÀ9´`ÎvñÀ;Àh‹Ô¡?èRßúÅ:@Gt.©6@‡¼Ÿ®·¿Ð1Ƽ›¿å¹6²Ää¿é÷ÏM
WŠ¿äœGãˆ?AGNfsrqTXS 1212+171?îÞñü>ñì?¦YŽ'\ù?¢à<áY?¦YŽ'\ù?î͂d^?»ÔrçA7?¯"'Ùº1?»ÔrçA7?ëz™rÓ?°ö‡–t¸R?©š4³À?°ö‡–t¸Q?ãÖ/?Br?Ã)Ð É¿²?ØS¡{÷?Ã)Ð É¿²3FGL J1217.8+3007@g›îàóË>@TƒDàá6À7i1"·ºíÀ:®•­¤é?å^·üŽ¹õ@Qˆ®d×Æ?ÿ—v~·k¿àÉø՜޿àDOÌಢ¿ßÃ`uiA@¿áùùšzAGNbll1ES 1215+303?ïýxå?¯?@×ÝÐ҃?48Ö‡å?@×ÝÐҀ?ïÌ!Œ{J>?†ÇpY‹b?yï9ÂZá?†ÇpY‹b?ïgõ¤g;?"­æSiÏ?"Ks"?"­æSiÍ?ïÞ@1KŸ£?nÜNw'ï?pßçZ0/K?nÜNw'î3FGL J1218.0-0029@qÖÿâ£Ï@N¢ŸÒ˜¿À9|Æ@Á'/À;sþ¨+¡?àÁ Á"—@··M^­Š@]a#Ü¿äóa£ý‡¿åjÊ!)xþ¿êGDŒ™Mf¿ÑºO­ÎkAGNbllPKS 1215-002?ïøéc"Œ?PüH«>?LZq±ÏŒÀ?PüH«B?ï«l'×¨?$€·ÖƦ?…$ÛXŠ4?$€·ÖƦ?ï,g}}²}?'a
|n(?šsPI°‡?'a
|n%?ï^,Á½"û?Œ¼ÀàíHó?":gÈM€¤?Œ¼ÀàíHõ3FGL J1218.4-0121@qà|`Ÿ@N5æ`ɊÀ9hq¡›À;`qå©é?Þ0$ðˆ@RìéLà-@Á?zê,¿Úà'yõíá¿áVzšÖ»¿æùïã&¿Ö·µœb)sAGNbllPKS 1216-010?ï(Œ\ë%? ØáÕÜ7?šÿ.tb›j? ØáÕÜ7?îñP¶Å?ªÀHó¹MC? êôžÃ¯—?ªÀHó¹MB?ëÆáíñ*å?®ÓŽ¦Í?ÀäxH;To?®ÓŽ¦Í?ìw@°'š‹?¯	¯·"F?¼Eú{ë+­?¯	¯·"F3FGL J1218.5+6912@_Ïÿ`Ï‰@GÑN¿ÓÀÀ:O…¯
À<îøp¿†¿e»_p_¯Ú@¡P&l@&îÿ|¢h¿ê³~ÁT¿çÚ:Þo®Ü¿ïª¦!ÅÖ¿ïí7©¬–AGNbcuNVSS J122044+690522?ïò¤ºæŽ?n'²"`ª5?Z¶Š2ãñ°?n'²"`ª8?í¿¥ö#?¿Ÿp
â"?·:ÐNçò?¿Ÿp
â"?î°aåèĘ?šŒ8mbŠ¹?¤ùá¡s¶–?šŒ8mbŠ¶?ë‹þw»ò?µ"w'š1z?ÁÓô!7?µ"w'š1z3FGL J1218.8-4827@r•øŸƒ¾f@,•"d~À9—æuë>¨À;…ª8MNg?ÃA¡b2Fœ@ÅUmðžc@°zÿzŸ¿á»Â/Ý4Æ¿âR1ÙR¿ã-1ò&µ¿ïäšZAGNbcuPMN J1219-4826?å±ÿ"Á¡U?Ê5ÿêê?ԜÖ|½V?Ê5ÿêê?ìpx>¡Ü?¾½Kh'•?¼|?æ
ñ ?¾½Kh'•?ç`Ìñ	èÐ?·?ВªzÎ?Ñ>fì._?·?ВªzÎ?ë¦ÍÐ;J?°2Ø5$é£?Ág¨È¿Û?°2Ø5$é¤3FGL J1219.7-0314@qù€#¦Î@MWý`OÀ9ÆÀâ³¾ßÀ;–ÿ³©æ?䓒T3'†@Á!ý*ãƒ@Ÿ§Ð"¿Öyw8':¿ÞU#ÁXØè¿à'Ž:ô¿âߙ
AGNbll1RXS J121946.0-031419?ïü? ô"[w?`b.J? ô"[w?ì"ÂÚ¡Q?¾)¶Ñ3•ü?»Ùé*õs¢?¾)¶Ñ3•ü?î:¯¾†=?žR÷½ç¾?¬_åœ,?žR÷½ç½?ä¢êÿ‰P?¸WÀqŸ8?Öº+öía?¸WÀqŸ83FGL J1220.2+3434@d^Õ•:@Sÿí ‹]À9à5"FK>À;éC¡É¿êÕõ7zÄ@`<O´X@oÿl\J¿áò¼:ƒ^š¿áËcÁ¤\¿äŠÝcÈÒA¿æàBÙL´AGNbllGB2 1217+348?ïÛM-­?u¢Ž`MÂ?rxYi)Á?u¢Ž`MÀ?ì™?—"ܱ²?Š¹þÓÙÁ?—"ܱ²?ï
"ç³ž?"(uÒæ?žMÃ	Œ??"(uÒæ?ïÕ[;×o\?vù'ă&‹?uRbHQ­?vù'ă&3FGL J1220.2+7105@_¢ïÝëÙ@Fè|à%o%À9Œõ#-+²À<|Ñâ¶C?Ò@XXå@ {KÆÓ@²¾ aŸW¿äII0[Ï¿åÁc"&¿ê"x×Æꤿè[ki;¥AGNfsrqS5 1217+71?ïüÇ9*‰-?CF›2?9Æ6«¶¡ª?CF›2"?ïžÅF@"?"¬†[­Ï‡?ˆN»®oß?"¬†[­Ï‡?ïx*½äy?Ž·¯‹¸3?ú®Cp–?Ž·¯‹¸4?ïÛ<ZøH©?kAsŠÂ¡?ra҃۫3?kAsŠÂ¡3FGL J1221.3+3010@gKØ't@T¯ &5À7É©f–7À:ˆ'–9?ٌ0¡Ð@Zys3~?úèÀž@G?¦cMû¿Û(ó/sû¿ÎŸ5åÀ¿Ñk…ÎÐK÷AGNbllPG 1218+304?ïüÁÜ\÷?@Ñ"۟Aa?9ñPGf?@Ñ"۟AL?ïÆ¿Óò-?‰š¹ÔÙG0?|ó éÃ?‰š¹ÔÙG/?ïX,÷ý?—Ù䜢ÞN?Ÿúa Q?—Ù䜢ÞP?ïÈy"…<—?zŠŒhià?{Ãn½a´µ?zŠŒhià3FGL J1221.4+2814@i5ÛߏG0@TÑî¿Ñ;ÇÀ7ÍÜcBÅwÀ;#Pg ¡?ëäb''k'@Fö¬o4@@Ñ£@Œb$¿Þ"yt51¿â'î÷øŒ¿àܽýôY{¿åXlR¹‹RAGNbllW Comae?ïþ$þz$e?+0÷Ú'9?-°]¹¬?+0÷Ú'^?ïÀ®I¢?‰[h7¹¨?¨Û8.òš?‰[h7¹§?ï"ÈxÆ?‡Ç-ÏQr?‹áùÎð?‡Ç-ÏQq?ï¬bJ昁?};aœ¬M?"çmFY߯?};aœ¬N3FGL J1222.4+0414@q͞?»×²@P…IÿþRÀ8Fˆ'
YÀ;I_ND0±?õ±Óšt¦@ôDÖÙZ@Aâ:È'÷¿åk´¿˜dn¿ê–î¼ê4D¿ìíâtåì?¿ÝÌùˆA­tAGNfsrq4C +04.42?ïþÎëG§?+á
)˜Ð?#K…ˆ.?+á
)˜'?ï¨]äªÌà?œ"}rDu?…è†ÕLÈ'?œ"}rDu?îà¼8nn™?—BI¾¬C?¡ô<yn?—BI¾¬E?í0}Ú'õ?°!¨PãÎ?¶|y.ÀU?°!¨PãÎ3FGL J1222.7+8041@_rÞCí–@B,Ò?ÓT¦À9+ªëÑtÒÀ;Ç«ZŒ='?×ي)(H@áuÁ"I¬@HÿÚÁ,¿à½'i›ò¿æÔ/[¿áå(­b3¿ê¸ƒÑJ#ÔAGNbllS5 1221+80?ïý´$ƒ?:s"2im?7Ú[öÛñ©?:s"2iK?ï$Eléé?š9Ò7®Y?›|÷RbÂì?š9Ò7®Y?îÕ^~6À*?—wmòÅí?¢ª"ýT?—wmòÅì?î¿éç†sQ?"æµ?¤a‡˜Êã?"æµ3FGL J1223.3-3028@r|˟ÛÒú@@‰`fr%À:vŽŒ]"À;¼ól|*?Âv¥´ì@
¼Œã¨±?þ/ƒáK‰ì¿ãšOˆ¿åüqЧͺ¿Ü
«±Ò©¿ÉW̵AGNbcuNVSS J122337-303246?ïþIVÆR'?.™ ¼pþ?+j"š×ٌ?.™ ¼pÂ?ïÆâñÕAÍ?¶¹ªÏÞN?|Ž‡_ö?¶¹ªÏÞO?ïÍ&}âµ?tî–"
ä?ylôÁ¥&?tî–"
á?ï½=Fþšw?x(a(ˆÚ?€°®@Yb?x(a(ˆÚ3FGL J1224.5+4957@`¼ÿÚ@S@P¥é`êMÀ:=އà4À;á¼é)ú¥¿Â¥ô*]³@L¤sgUÐ@´¶ŸcÝö¿âµý¨ëNÌ¿ë'Éùkø¿Ó7"E5­ü¿ëôHÖAGNfsrqSBS 1221+503?ïýA##ˆ??@‰…YÛ8?5öæã¾ö?@‰…YÛ3?²-?•&ñØÂa ?ˆÓt¹	?•&ñØÂa ?ï"!ÓTâ?‹úËÃ4?Žÿw‹*Ç=?‹úËÃ5?ïµ®yz®µ?yÖ
	X?'"a¡TRé?yÖ
	Z3FGL J1224.5+2436@m@ôŸM¡@Tܸ¿ÏŽHÀ9†_:øúRÀ;ˆ›†Ù£?μÛÙì+H@𪮔Óa?þ0é
ìî¿éŒT¼ð¶·¿Õ0yשÁý¿ÔûòÇ)¿ãπل@AAGNbllMS 1221.8+2452?ïøÞñ,´?K¯B§Æì£?L‡ì;M1?K¯B§Æì´?ïeðl6k?ŸâÚ&ÈÌ?"Aý²y2"?ŸâÚ&ÈÌ?ï [ÿ"b?'è
¬?Ô?‡üé7gv?'è
¬?Õ?îË+Ⓓy?•õª'FÈ?£MAÖÔh?•õª'FÈ3FGL J1224.6+4332@anýæOU@R-‹àôÀ9´Rb£cGÀ;ÿžÁ÷†µ¿àºñQ!ÁØ@­á­.¡Ô@]  Ö¿æh¨µì6¿è õ(¿Ž¿æW|ûBð¿ïÿ⾦™\AGNbllB3 1222+438?ïþ¬mãop?'—¢™?%9!É	
M?'—¢™µ?îýºË†Ë?ª"`H"? $SH"S?ª"`H"?ïz¹ÖW?†Ö¸fx?ˆ¹aQŠjE?†Ö¸fw?ïeêߣ8?<eæ;+Ô?"\B¤˜ö?<eæ;+Ò3FGL J1224.6-8312@ráoŸËÀ4a¦¹Ù«À9zeÜÓ«
À;{ ù	kº?¹3ݕ+}@#ÏÃøõ@Ž_?«'"¿ä‰'å´g¿êj\´Ù2ƒ¿ãü¶Ôâm¿í|3FUAGNbcuPKS 1221-82?ïàe÷pæ?§ˆ8Iõš€?ãóAã6?§ˆ8Iõš?ïM¹GG4¶?¡(©¹`?–H×iB?¡(©¹`?ìbw˞?°Rn0œÔº?¼ïç,A£	?°Rn0œÔº?î½ü­T2?'‡ˆ("v?¤ 5.ª¼æ?'‡ˆ("v3FGL J1224.9+2122@oáç_ö	Ý@TjV ŘÀ5û‰SÑ8lÀ:e~ƒ"×?ù»]¹™";@#šŽSz@ñcá¦Î‹¿á"ìÂû+Ÿ¿åOA
çIP¿äÔ]X†åô¿çH%p|ê·AGNFSRQ4C +21.35?ïÈL,®Tý?‡+m–šPü?{Ùé¨Õx?‡+m–šPú?ïÙé;—t
?'Æê34÷?sb4EùÇ?'Æê34÷?î^®/çãú?¡B++R—?ªÀz?¡B++R—?ïÿÿ۔w×>‰Cž-þï>r5Äpo>‰Cž-þ· 3FGL J1225.7-7314@rÐÛ«–òÀ$íG¾Ûr'À9á¢!þW‰À;s`c'¿ò©0
3à'@>}[ËWØ@y¬ÿ§ël?çöE€‰q¿ìãrÜÁ¿Àvö%$–|¿çã•&ÔfZAGNbcuPMN J1225-7313?ïû4ù)¨Ö?Iª6øãZ%?C,Y\¦–?Iª6øãZ1?ïƒb¬Š°M?™Jü7æ?'TÝSí?™Jü7æ?îà
ãÂx™?˜]?<€n›?¡ÿ!ÃØvq?˜]?<€n›?ïþS‡Œ²æ?14´?*LJ4ё4?14°3FGL J1226.8+0638@qÝõ€í @Q,ڀ¶–À:ámmÁ¤À;·ÉjA½:¿ÔôU–¤6@
‹w+/®™?ù>ÎÇÏ¿í··pˆíê¿ßø…Š…Q?ʦ`;ÿàu¿ÕS{ìÏ:AGNbll1RXS J122645.2+063906?ïþZËç?4Ýø.ô?.ÊSAŽÚŸ?4Ýø.ô?クgù‰±?ŒpŒ:™A?€'æ"é?ŒpŒ:™A?ïNNÕ‡Ù?'wÇʪ£d?–6%G¯?'wÇʪ£e?ïÜDääõÎ?~¹¤ݸ–?qݍ…Ü?~¹¤ݸ–3FGL J1226.9-1329@r]®@…+N@Hxwò
ÏÀ9.x,a‡ÚÀ;R½¿Ïæ?îƒÝy\&5@KŠó8œT?ÿ¹V  žñ¿ïþÞY‰€"?ïèÏ;*è%¿á"30¦]¿åY¬µç´AGNbllPMN J1226-1328?T1®â?"³X§Q6=?‹Tjó"G{?"³X§Q6=?ázcÔyŸï?ÓHëÚ|?Ý8WÀ"?ÓHëÚ|?ì¿t²:<ý?¦c ó-`?ºZn.?¦c ó-_?á_6,IR?ÄßV,º†ë?ÝA"§mÙ]?ÄßV,º†ì3FGL J1227.9-4854@r¯CÀ~à±@+"É¡Ÿ!™À7蠖ãÜ´À;ϹWf?ø‡¤Ò1æ'@Džïnã8@–5¶ñ¿âZˆKµØa¿äP¡KÐÊ¿çü?^Ã8¿êßÿ_PSRpsrPSR J1227-4853?æÄaÐ}Õ?Éxâ'Ú?ÒwÏ<_U?Éxâ'Ù?½ñ¹zGì?È[d¾'³u?ìAßhз?È[d¾'³u?â üdXM‹?¹L 2Úõä?Ú¾7Odé?¹L 2Úõã?­ï6>n)²?—úp¹ü?î!œf?—úp¹ü3FGL J1228.7+4857@`™¥ 8L@Pî‹î²ÑÀ9èûŒ3€À;©ÏŽH,¿¿Â–Lwg@á©Ë•ë@ë€z8Ö¿äVˆ: ¸1¿äS‰ëY]r¿í94?*jë?Ì9¿ãǪAGNfsrqTXS 1226+492?ïýöAû?5ä	Øg?0Oý÷h1C?5ä	؇?ïÒÁný¹Ð?"ˆ‡ž†*­?vŸH#B?"ˆ‡ž†*¯?ïs&E`Ƕ?ŒžªH
¯?'›7Sç	_?ŒžªH
¯?ïö"/R¤S?TåñʑãŠ?R÷¡Z·Z{?Tåñʑã"3FGL J1229.1+0202@r¨@[9â@Pr@#Ü~À6nç=À:Üš\78?ÿ£"¦%@!ñ@­DFV@Zâ"o¿å±*SrÁ¿é8÷(JL¿êjÏÃ2€l¿êw({Y\AGNFSRQ3C 273?ïô ×w§}?ZSë†`°«?W¾Q±X?ZSë†`°¯?ïÚ÷8yþb?ƒL‹'Î?r"cÃι?ƒL‹'Ï?íHþœûh"?¤0‰|«LZ?µ¸$»a?¤0‰|«LZ?ïÿõ¦èk>ãr¦Ü³x>Ô²/ß)±Õ>ãr¦Ü´Ã3FGL J1229.8-5305@rºm ‹]@#H>¿ÙI]À:;zç&ë&À;Žã©8?°V)bßO@5Ãm}†é@,àŸ©¿èohÚ£¾Ð¿ècVX.ª¿ÑÙ9x'ÙË¿à`Á`¥AGNbcuAT20G J122939-530332?ïÿ;lê%?{}~`Å?Ÿrb»RÓ?{}~ai?ïÈz?Š½k?À–s·]$?{Âà:¡J¾?À–s·]$?ïçæšÃ
ó?m¸{Ám…?he<ò
É?m¸{Ámz?ïìí@˜?\ώñ^‡?c~¿üg¯?\ώñ^€3FGL J1230.3+2519@mF`¢G@U;{ îÙÀ9PY´§<À;Ÿ"ËÜâÅ?é¬^U©]e@:ä1Bm8@âàK¯¬¿Ðad¸«'¿å9ýgIeO¿ã߃ÍnL¿æ-b†Ì§AGNbllON 246?ïþê¤rÿ¼?-‰v W?!U¸ÐC`?-‰v {?ï|ól2'&?Ÿ¥Kúi?a'y»,?Ÿ¥Kúi?ï.ÕrÔSŠ?'z¹ãH?š%Q¥uŽé?'z¹ãG?í¶-=ºÅ?¢ªàìa‰?²N—)Ú?¢ªàìaˆ3FGL J1230.9+1224@q½lºËC@R ÂÀ®À8ô>A"/À;c‰ì}l<?½óg¥<@ôÖÂ@R`0lY¿Òð‰«öú"¿á/¬i0Š¿ßÝí3¨,¿éÅN>b¢AGNrdgM 87?íæù¾Ãš?²*ò^Mï?°È7B	ã0?²*ò^Mï?í£t°Â8?¶7'Ûõ,?²äZyë~J?¶7'Ûõ,?èŠO*ûf*?µLBß]?ÍÖÃTg]?µLBß^?ì|}#Y³Ø?°&°ä
Ò?¼å2aE?°&°ä
Ñ3FGL J1231.2-1411@rxž?»×²@H1ÀY!À6ÿcëaãJÀ:á\·ûe@	dŠ÷t@DETH?ûšÞ˜–?¯ñO8!"Š¿Ù|µ^C¿ãV^´ó¿í«Kô±S†PSRPSRPSR J1231-1411?Wó(Nçô?Q=Ó<‰Ô)?ïôuk؋?Q=Ó<‰Ô)?Á¤¿ˆ›Ö?¶EÝÞDeE?ïyòÚ»!?¶EÝÞDeF?¶îbœÝ?®É‡ãâ&?í"3½l}e?®É‡ãâ%?.Hu?ðô5Sèa?ïÿ¯G¾ß±?ðô5Sèa3FGL J1231.5+6414@_ qÁ
{ê@J`»oÀ: 'oÿl\À<PœÐ…¿?×Ì°áù@2ugMA?ÿwß	»@¿¥' x'Û¿×PÈfØôp¿ç;Cɔš=?Æ4U-j,«AGNbllMS 1229.2+6430?ìcòOy¼?ÀÓÜô¶ç‹?¼àm"2D?ÀÓÜô¶ç‹?ï]¢Ál©?žæ…0÷–?"K§ÜÒjÅ?žæ…0÷–?ì9gE–¯
?±4p §Nä?¾4ÅÓJ‡¸?±4p §Nä?îðÓéüP›?™}ÄٟC)? òÁ`:öQ?™}ÄٟC*3FGL J1231.7+2847@gÙü?O@UV™¦5À82~5ÅÀ;
3Ï:eW?ã쏪yÞ
@C¨×¥ý?ÿ-À"!¿ÞÁ¼š½ ¿àÞúvÔ¿Ý7ÁÉu¿ßÃt|9óAGNbllB2 1229+29?ïý)Ûbýa?9Ö(/–B?6±$èòE?9Ö(/–Y?ïÌ6ú%æÌ?ˆ˜©Ë™	?yä'í™é?ˆ˜©Ë™	?ï®#&cÀ&?€ó"8æG¤?"w6gö]?€ó"8æG¥?ïÎٞ`Â?pȦÐ)¹n?x"0ÏùŸ?pȦÐ)¹o3FGL J1231.8+1421@q¤˜ˆv\@St÷íÀ:,÷öFBÚÀ;¼ùS="¶ÀŽ_¡¦-|@4Ö8±Li@…=ÀªÕ¿âqõ!¿ä+t¡´è¿ÜŒBX•¿äҏ™AGNbllGB6 J1231+1421?ïÿv«4Ù?®â/G2?q*™e'?®â/H5?ïÛÀÊbƒ?€WNHºq?ršÎó½þ?€WNHºq?ïº2qx?;ãÕÑüb?~üóc¡Ì?;ãÕÑü^?ïÿµJ_pæ?ZÆFqÄÐ?­h#Æd§?ZÆFqÄ#3FGL J1233.7-0145@r]cÿï9@Nf­ _À9úö«ÃhÀ;{µò•´?ÙÝW^‹§@üsƒôl@ÅhpM›¿åÚ¯/û<Ä¿ã<A"<ɿ㖭gÆ|•¿ÒÏç&×AGNbllNVSS J123341-014426?ï¤U"Â?‰ö{•º?†ù9ª›5?‰ö{•¸?î9õ+?ºO'·8ž?¬o0¯}N¾?ºO'·8ž?íÖGÄÅ»?¡nÝÉ"Ká?±MÁÙÒ'è?¡nÝÉ"Kà?éDƒÙÝý?¹ÙTii'?Êíóܘˆ
?¹ÙTii'3FGL J1233.9-5736@rÉf?šIÃ@½ËCòžÀ8ÊÅ­ÚÜÀ; Îô©‹¿ðØOÒ¦*¢@Aˆ£¨U@Pèß|ý­¿æ¢.§n¡¿ÞèžÞä
¿âÿÉjä¿ÝE?IR@AGNbcuAT20G J123407-573552?ïã¼BZù?eè'SZ?lëC½¥x?eè'SZ(?ï»d²Š/?yÍ?r¡?&Ó]t;G?yÍ?r¡?î–GR?™†>Ó ô[?¦žŽûŠÖþ?™†>Ó ô[?ïœ9?aýÛ¸Œ†?awwðcÇ?aýÛ¸Œƒ3FGL J1236.6+3901@a&°)(@Sm~ßÙïËÀ:~1«s¶±À<
M`Ûã?Ä¡‹Sc\ú@0"[—*@ï·¿ttœ¿îFK­—A>¿È:́ʿã—e{ž¡¿Ø2Ÿ,´¯AGNbllRX J1236.4+3859?ïÝl4ÞÙª?€"¹¨jE?qI吓+ ?€"¹¨jEœ?ïr½		Íä?¢H&"/Ë?'¨^ÞÆCG?¢H&"/Ë?î‰Â©$Û ?¢1CQW W?§cÕm²Mý?¢1CQW W?îìæÒ¤r?—T·?b7?¡?ђոÒ?—T·?b73FGL J1237.9+6258@_b^AÔ¶¦@K
q VL=À:Ƽj~ùÛÀ<+Š«ÀË¿È;Ki¤£'@% ¢!}~?ýb
Cœ¸¿ìُ&_K{¿Ù¨L·"«¿Ön°Ëu›¿ÔlZÚàaAGNbll1H 1241+626?ïÈoNBÅ?ï¶@r±?{ÈXޝ~_?ï¶@r±?ïJ\þ'W
?¡,Æðøù–?–´`;µ?¡,Æðøù•?îA
™^rZ?§
Œ5+J÷?«ïVjÚW?§
Œ5+Jö?ïŸB¤ˆDQ?'4¶¨Æœ?ˆ/VÝîë¶?'4¶¨Æ3FGL J1238.2-1958@r«f?šIÃ@EcêßÝJÉÀ9¾RsjZèÀ;´'¾ÙÅ?ÖÍ25K*@)ìþñb-@ÊÀYY¿éå-¤Òï¿á©ÉÆÍ¿Þãµ¼ºÛß¿ë¿öAGNbcuPMN J1238-1959?í=;ì,?¶FÀ9¦»Y?¶ ŸÖŸ×?¶FÀ9¦»Y?ífßÛ¯ƒ&?·ÄîT†	"?´É"ƒæÓ?·ÄîT†	"?ìøCu=?®§yjF\>?¿@=äS~?®§yjF\@?ì^PCÖ®?¬¬ºÙš¿R?½
}çáJŒ?¬¬ºÙš¿Q3FGL J1238.3-4543@rÈÇ`|Aš@1cÀ™¸£À9Îä¦f&À;©:}ªP¿ï™£ÒO)@|b¤dùª@9Ê?©¹!¿í¿:ÓI?¢‹ºÖ!¬š¿à'n¦`ý¿åÔórFfAGNbcuPMN J1238-4541?ïüµl}|?8Q)=ÄÞó?:TœMÈ?8Q)=ÄÞí?ïÙëê}Ø|?ç1Îæ‡?s

ÁÁÍ?ç1Îæƒ?ï°)
í©?"|sí'?ƒÿu¼"•Û?"|sí–?ïúº©ÞÜ?F{¯]îË?EX‡ô‡Ò?F{¯]î½3FGL J1239.4+0727@rc}sÉ@QˆfxÀ9½â¯ åÀ;§†_*2¿ñŽÑú‰ @j«Yàq@.Bß·7¿éÓì$<0™¿á@­åßuú¿åì''GK¿ã¤	"AGNbcuPKS 1236+077?ïÍKO¦÷S?€C"'Å.²?yZX,"Vk?€C"'Å.µ?‡±?–èš'›
?ˆýÞ›ß?–èš'›
?îp—,v²? J¯¥ÔÕ0?¨ö7"Ñ? J¯¥ÔÕ-?ïékpË»¯?fÌKù`aZ?f"4DO?fÌKù`a_3FGL J1239.5+0443@rs‰ :2+@PÚqÿ÷œ"À7'Œö(/À;¢!'—ô?ûuëæmˆ@ŒIõl~.@í*#•‹¿ágï¨nô¿å¥9¤¿æfâN3Œ¿êîÀmvƒžAGNfsrqMG1 J123931+0443?ïÓ#úîËt?tMµbÅ*Ë?vnˆšF?tMµbÅ*É?ïÓ4Õ®`?…ð6·–óÞ?veü•(Ðá?…ð6·–óÜ?í³7¦à?¤Äû+»õH?·¢fBÈÿ*?¤Äû+»õI?ïü-^J%Î?A¶¨N=}Ð?>•
®Ñ‰É?A¶¨N=}í3FGL J1241.6-1456@r¶a_Ìr@Gíù?ò^WÀ:C5'Ì÷À;Ækš'Í¥?â'AêÂ<a@º¿-§Ù?ÿYÊÿ˜&'¿îhŽa'&?žGь
v¿Ôyµ€¸Í¿ãé<¾5AGNbllRX J1241.8-1455?ïÚ'ÔY>?zãÊò?róìÓa-?zãÊô?ì°©Ì&p?¶ ¢˜ß?¿¢z±žÌ{?¶ ¢˜Þ?ïOÁ'œâþ?‹ÌrÂèçÊ?–ÍÌc H?‹ÌrÂèçÔ?辺+ G\?·Z²KÉUÝ?ÍQ~â?·Z²KÉUÝ3FGL J1241.9+0639@r'øÿûÎB@QZýç!À:{õ[aO¦À;ÈÎX%[?áTr^÷Å@^wڂ?üÄþÍ%?Ìqƒ£Á™F¿ê'äjÎ*?¬`Ÿ…ŸoO¿×åï!z=AGNbll1ES 1239+069?ïý¼Îò?5üõAÝî?2!ˆkÄ?5üõAÞ&?ïÈjp³ý?‰lǬ³¡â?{ÊǦ•?‰lǬ³¡á?ïzq²õ?‡s]¨æ«ˆ?¿±É¡\g?‡s]¨æ«Š?mlF]'?1t+YØÉ?€œ¤îhŸ>?1t+YØË3FGL J1243.1+3627@`¡aՈ]@T Æà#Á¦À8i§e47?À:ùP°ò{³?ËQcøšÓ@@쉫æ?üM$þçüÿ¿Ý£!%G?ã¿×¹O»¿ØZé[!ܿӕ¾ùiRAGNbllTon 116?ïõ Už¨Ü?U}Ò
ˆÎ?T¿T®H½?U}Ò
ˆÖ?ïªó"ü*V?–H‰•Õê?…C7@õj?–H‰•Õê?ïƒéŠÕÒo?Š)óÙ¤ð(?J‹dk?Š)óÙ¤ð.?ïDœîãi?Wj9É-5?—lb#ž"6?Wj9É-63FGL J1243.9-0217@r±µß덂@NDÿ΁ÙÀ:L}qDçÀ;Ð:FLëk¿Ç­Í‹Â&@t¿CLZ÷@|Ñ`…Pâ¿çùÄ­ù¿ÞÝD3[¿Ó½°"퐿ê"ìiSAGNbcuPMN J1243-0218?ïQßÎÏ°%?œ4gôrG?•Ä&	ûe?œ4gôrG?ïs˧M˜«?—
ó
¹F?'†‹Lê¥?—
ó
¹F
?íbÙh`?°þIüß?·Äïi4½?°þIüß?ìR¤?ƒ©‰ùW1?‰˜Äÿ«V×?ƒ©‰ùW13FGL J1244.1+1615@r\:¿¹¾Ó@SÀW_ÍÅñÀ:6—ºœH¡À;Úe€…¿þ˜óï{xq@fÚ`´Ø@i1€«Œ
¿å±‹I¹vH¿äú–wâJõ¿ã*0¯dÿ¿ïÿÔ¸àÕAGNbllSDSS J124444.35+161621.7?ïý³àÄRq?=Þ½Éb¬,?2`ùÝlrã?=Þ½Éb¬)?ïͯש?†ªþV¾?yw@(+›?†ªþV¾?îá¶[Ÿ‡?˜'&þ?¡äšFŽ>?˜'&þ?ïþFŸG?9-¹S˜€¾?+ž/F…¨?9-¹S˜€Ñ3FGL J1244.3-4955@rÜ7À*ýÛ@)ÛҁA³ÿÀ:vãŒ+óÀ;ŠW™¿Ã?†Š•'@o"9櫛@{ÿªÅ'¿ê¥¸·Ó&¿¿æ[±9'ó¿àÃùòþB¿ÞIî±##AGNbcuSUMSS J124422-495422?ïþðe¹Ûà?!QÔÏדØ? ù¤bB$?!QÔÏדÒ?ïюV v€?û(bCC;?w8Ô¯ÄÀW?û(bCC7?ïÔÊîö—?sÖqʋÆ=?ušˆ"´~‰?sÖqʋÆB?ïׁζóÛ?h¢Ò¦áÞÁ?t?¤†!?h¢Ò¦áÞ¼3FGL J1244.8+5707@_. {5+@Mýþ +ïrÀ:PÃë|»=À<¸e6»~¿ØšËOkšz@(=}¥@½?fj¿å£éqè¿ß öÍ0 ¿è½)¼<ë¿¡X\|F'AGNbll1RXS J124510.5+571020?ïNŒfV{D? Fµe6ª?–.s50—Q? Fµe6ª?ïp`ëɀ?›³õC›ô?'óý¢†Ð'?›³õC›ô?îgGÓa?¥ždœÔ%?¯Ù‹'ÏÙþ?¥ždœÔ%?襁xY?'VÊÉ?…Ra鹝?'VÊÉ3FGL J1246.7-2547@rÙÈ¿Â"O@BˆÄ`Á
À6þBÍ*1À:Ï;+O9#?ûpF™ @"±M?@ŒL/Ùa†¿ànK¾´9¿ä"ö•Ú-š¿å˜©PŠ Ç¿é+=}[lÛAGNfsrqPKS 1244-255?ïÄs¡H?ztV"òz?}Æ1/~Ûp?ztV"ò|?ïÊôÒÿ'?…]ð§¹j?z…–€7y©?…]ð§¹j?í;§ ÒÊ?¦cC"	ƒÇ?¶"ÂÿYi¨?¦cC"	ƒÆ?ïù\4DèÅ?P'ÀáB?J.ì\å€?P'ÀáBŸ3FGL J1247.0+4421@_fwž™@R0Ÿíp±À:šF…öN¦À<^â
¦²?í¯2½T@7—›è~@wå¿·æa¿æ9Öi>ï¿ë¨6ýHs?»(8¥°K¿Ó7âÿÐAAGNbllRX J1246.9+4423?ïÿZ»
–?àDU÷aü?¨žM?ek?àDU÷b"?ïÌÃa–<©?†è+?yžO4á«E?†è+?ï'*OÎ?—ndõ¿?›½vX?—ndõ¾?ï×Qo¡Ã?{;åUq¨'?tWHv/Õ?{;åUq¨'3FGL J1248.0+5130@_Ž`€sX@PgGÿÞrÀ:"HÊt,ùÀ<­»§¿êç
`™P|@ç	ç5@N¸@xÁ¿ëiĦ¿Ò|ҒÎ=)¿â&|§­¿ç©	¦ƒAGNbllRX J1248.4+5128?ïõsGg€?aUÿ)óžÅ?Uq1ÒþP?aUÿ)óžÊ?ï·ÕcŒËY?–… é?'
§Í)ˆ?–… é?ï-é"Ör?™"^³ö^?žšBÏe1¿?™"^³öa?ïðÈ؞?`Ók˜ªþ?_ÒoØNż?`Ók˜ªþ3FGL J1248.2+5820@^îÊâ°@McC hÀ´À7Òæ±z`ïÀ:ÿÕHœQ?â"èç#~ú@µO{é/"?ÿ(«Àb±%¿Ü1\~†Ý¿ßԒ;ßÝ©¿Ý…9ÿïÓ§¿Ü½œóì zAGNbllPG 1246+586?ïä»Äëõý?uÊ Oð0?kD;
›?uÊ Oð0?îZ·ðæ.?³ð'n±¬?ª_4€ñ?³ð'n±«?ï0ti\Ð?—†m4Œ®?žyñrÔeï?—†m4Œ¬?êh󺣫Ó?¶íAÝï3?Æ\1qP´?¶íAÝï33FGL J1249.7+3705@_6ÆÞvB|@Týß=À9³ªŠ'¥aÀ;m¤K¤CA?ñ-
¦®*@—üï)n?úx@HŸ¿ïÿÒ~p&?ïÿ#Ý"¿Çzß¿Û­KÄ	ëÍAGNbllRX J1249.8+3708?ï܍&ñç?tGÖüWb?q¹tì‡?tGÖüWb?îíÅPÿ'u?³ïEÌ5X±?¡#ªðØ­?³ïEÌ5X±?í|£RÈO?¤m•h~œ?´åi¿õ€?¤m•h~œ?ꯁƒ'|÷?¹B²(67?ÅAùñö&?¹B²(673FGL J1250.5+0217@ræÀ]RÁ@PJ¹ßõž}À::¬¤8À;²I|JÔ:¿¿$b#ÐXŒ@Nò^@Ÿž¿ô!P¿äF+"Eӿ祐¾¤¿ÞmŸÌtÉg¿Û#Þb\§²AGNbllPKS 1247+025?ïþ݄"?2ÕÈü´y?.ò'¾æè;?2ÕÈü´m?ï°þÝJ2#?'S\YSƅ?ƒÀH­sw¡?'S\YSƆ?ï£%Ñ9t?…š«Lb?‡6‹±¢úŽ?…š«L[?ï½ýs(ë?ulùæ€Ë5?€€£5Å;_?ulùæ€Ë53FGL J1251.0-0203@r뿀ß×@NhP`j£ãÀ9Ûs"u"*À;²7_ÞO?ÛdÚ¨¶ @&°™_^@ùf!È?í£Îxoê¿è±úŽ|¿æÆ÷ ¶¿æ¿Ê+€ÚAGNbcuTXS 1248-017?ïÿ6£{	?r:ÄUÌ?+ŸPž¯™?r:ÄU°?ï²|"Ìõ?ŒrL—/"á?ƒ}àÞÌŸ?ŒrL—/"â?îáX=1ëà?–!ÈQÚõƒ?¡ê|,áB?–!ÈQÚõƒ?ïœ^rƒ?€Í–¢%s?ˆè#z߯?€Í–¢%q3FGL J1251.3+1041@rî-?ž{@RcÒtwÀ:ä9ÐÜ&À;ÃSP	,Ï?ѧâõ$§!@ÿ™©ß¸@'‡?Ïε¿êiMk¿çõ'C‰¿×.FíØ¿¿áX•:íÅHAGNbll1RXS J125117.4+103914?ïÿáÿ†y">îŒ(0;ìÍ>îy†ÞW¢>îŒ(0;ï¯?ï¾s2ízk?ˆÃú¶°?€c3D¡e?ˆÃú¶­?ïà~Šé†?t"Éôp)?ouùz?t"Éôp?ïÒ%ûþd?jåÑÚE}æ?víÍý¢?jåÑÚE}ë3FGL J1253.2+5300@^"®ÀrKw@P9ßõž}À8U'ÙŒÀ:Û«8þNO?ôE!óé@µ¹	÷P?ûæÁšê|‹¿Ö×,>CÔã¿Þhvšò¾¿Þ}âw­¼¿ã8á…ÁuAGNbllS4 1250+53?íÒqµ¬?¶ÌyaËoõ?±orRŸ'?¶ÌyaËoõ?è-^î[É?̝ÀÃÅV?ÏJ"FÛÆ?̝ÀÃÅV?êzå£Á]?°&ëú=ób?ÆipúŒ?°&ëú=óc?×y⚽c?½oP{9 ø?äCyŽ²¡O?½oP{9 ø3FGL J1253.7+0327@sп "`@P•€	¥›À9o™YعjÀ;^}Vlô¿ñdt
Ãâî@–«†ñÌ?ýwý%	O¿ÐV>Zø¿ß-‡Ç#¿ã,tè$Ë¿Àº½mU»@AGNbllMG1 J125348+0326?ïñ¿Hµ-?bÏðÿ\¾?\oĕ¦=?bÏðÿ\Å?ïÖØ-÷ŽÐ?†Kq»½Ô?t"é8˜?†Kq»½Ô?îþ¸«en]?–_²]»K¸? uI©E?–_²]»K³?ïþÿ¥?1uæÅcR
?.^0µ®"?1uæÅcRG3FGL J1254.1-2203@rüÀ?ö@Dg_ !¸À9¶ôöºÀ;"žý†¨ü?ÖXâíþÿ-@¬ã £Îý@]€k_ʿݔûùúÇ ¿æ1Æ=³â¿ä~ùlóà¿à^¬
+AGNbcuNVSS J125422-220413?ïÉ¡–í)?¦y!:¬£?Ÿ&ËÍ"Zæ?¦y!:¬£?îªÊ:Šu?«'GÇ¥uÑ?¥S\WX®°?«'GÇ¥uÑ?íÀáö>q.?§ánWÌŽ?±øðNv‹?§ánW̏?ìâñ©¿Ëø?¦˜£j¥ÒZ?¸èr² G?¦˜£j¥ÒZ3FGL J1254.1+6240@^™"ÿ‰;@K9R¿ÀtÐÀ:†T‡@сÀ<€­9‰?ً€/ÿæÄ@o5w±…?þo'ßì\?ïÛýž?µf¿»w?"e쪿â܇hGDÁ¿Öº›¡ŽªAGNbll1RXS J125400.1+624303?ï8QÞL7?§ÀòÄgò?˜õÄ<–y>?§ÀòÄgò?î¯câ0¬'?²¹7â†Cã?¥	ÁÜõ6é?²¹7â†Cã?íœCÐ??­ûIó²x?³á§Î?­ûIó²y?íËȒàt?¨d•NÇt?±¡Û›hüX?¨d•NÇt3FGL J1254.5+2210@sr>À¨@U?Ô ÄÿÀ9¹âÅ\–À;ªw"^?äxg¯*"B@
¹sólÉ­?ÿî_a9€Õ¿è	
£_I¿Äò}¼Õo¿Ý­HTúÑ¿âi°IsšAGNbllTXS 1252+224?ïà÷Hƃ\?sþÂ-‡¿"?o·9|¢£?sþÂ-‡¿"?ìgÍγF‹?ï˜ÍE6§?¼Á'Še˱?ï˜ÍE6¨?îßÕØù6ü?•ÈD¥}Å3?¢¢pl2?•ÈD¥}Å3?ãk >?Â9½ÿPÃÉ?Ù)¿Õƒçß?Â9½ÿPÃÈ3FGL J1254.9-4423@rùŽ?þó'@2yMŸÆ…À:[®UéAÀ; þ"ÅõB?á¦Ä'6Т@
vêb^ïÐ@Žâà_{¼¿çlXç³ê¿êÀ긽¿ÓÓàò'¿ÄvÛ">ÝûAGNbllPKS 1252-441?ïû½XHu:?B¢"HwKI?A
žÞ+Ù?B¢"HwKN?ïÆî-¥ñ?";Š]{Cî?|ˆéw­:?";Š]{Cñ?ïjˆýç'?s™a÷X?'®ÿ C•?s™a÷V?ïm»¾®&²?‹½4Ð˜›?'Hˆ*;)Ô?‹½4Ð˜š3FGL J1256.1-0547@s†_•'Í@L‡Ã¤àõÀ6'_Tú-XÀ:}Uü‹×9?üãv$˜G@ ¯X	"µ@WæÄÊ׿â[#&9"¿æ.>¦Ñ2¿åHסßZ»¿ç:àH!#AGNFSRQ3C 279?ïЩ=åЀ?~³¢zÌS?w«a
À[?~³¢zÌV?ïÕUeYØi?…H1--):?uUMSËN?…H1--)8?î}¾†15? 	kòòñU?¨."œì¬? 	kòòñT?ïÿÛÇìéÊ>þ$'õòu>ò	‹TÚ>þ$'õòj3FGL J1256.1-5919@røœ fè@VàºÛ^À92ÃWÙéÀ;Üæ"*¿É}Y†.-@5Í.œu—@X`d¿ËSiè½'¿éñX±¶µ£¿ßÀýFùIê¿áy³¤rAGNbcuPMN J1256-5919?ï²tp܀u?¤ÀÍùú°?ƒbãÈßâh?¤ÀÍùú°?ï{&¥…´[?œÎ9¨ˆÀŒ?›+OIt›?œÎ9¨ˆÀŒ?íÜí?=\u?£ùˆ"Äòc?±–V?£ùˆ"Äòb?ï}I•¢ 7?…¿JA´_?VÍK«ù?…¿JA´_3FGL J1256.3-1146@s
…ߨq¤@I‰L߬£bÀ9—RMª­¾À;|ë Í¿Ÿñ|Êúç@Vô™špY?þƒ %"º¿ç³֎Ë¿Ô½Û Ø°¹¿â-ßÐúH¿ÄXPüXÅAGNbcuPMN J1256-1146?ïü™wf;ƒ?E€š¨õMÞ?;4DÎ#ݔ?E€š¨õMí?ˆ?_dß׬E?‹Rþ}8¾?_dß׬D?ïiPåsû?‹uõ?'ÕãQœ@¨?‹uõ'?ïÓ ?p¨ÖQ·`›?v£s«/´?p¨ÖQ·`ž3FGL J1256.7+5328@^I' ÿT	@OÒŸá²7À9Ñk÷Ÿß.À;'l	=–d?®÷û¸hSá@šZ]n›@ë@UZ¥¿ãì…g]‡¿êBÔíÇ]¿ä[D,L1¿ïÿåV9%CAGNbcuTXS 1254+538?ïþÇꮜ?({Lɶ=i?#ŽaU[0?({Lɶ=,?ï:2س?£43	8l´?˜¹¤üÝ	?£43	8l´?ï–ð[ö¨?‡57oÍ?ŠCéUÿO?‡57oÌþ?îik­ÊR?œê,~ÐÊw?©iNu#ZÝ?œê,~ÐÊw3FGL J1256.9+3649@]×®6	@TUÀ%õ]À9 /ªèvÀ;Áڅ4?C%҄@¸'ô´@¡Ë`;)!¿Ývƒ¢êÙ±¿àÝN,çGU¿ãÇÔ©©Ì¿Ú"0žÙIˆAGNbll1RXS J125716.0+364713?ïöÁHE'?aÙ­b/ʘ?R}otÛàØ?aÙ­b/ʛ?ïˆe"÷êÃ?›üˆÎ,Þh?æžÂOŽ?›üˆÎ,Þi?ïƒCŸ|?–¬:÷ˆ?¯—ŒЋ?–¬:÷ˆ?ï;Ë2K·?lµ©i?˜†œù¶‰;?lµ©i3FGL J1258.0+6120@^`Ú¾'œ@K─U$öÀ:ÒÎX%[À<C"]È23¿êó"Q'²C@
Ì\Xp"@ÅQ *­¿ïŒ ÈÊ?Ö¥™§±_^¿Úøj
›ö|¿ÚKàZÀFAGNbllNVSS J125820+612049?ï¸ÃÅޑâ?'—ãá—?Ïˆ[‡ô?'—ãá—
?ïù8>õ`?'jáû™™?ˆ±ðB¨M?'jáû™˜?í‰ëÖu?­‹öøºš?³°¡OüWÌ?­‹öøºš?ïóñ† ðf?U›YçÕMZ?Xó¾5:?U›YçÕMQ3FGL J1258.1+3233@[±þë-
@U[íöéÀ9‡"¹À;ÄnŠ!V'À¸gÏ2f@€2t†@»ÓÿÆõ¿åsôwek¿éÂÒ¼¿¨¿âšâ™èŸ¿åL?ôŒ¯AGNfsrqON 393?ïÿòæρ">àO»ˆ\!>Ú2`ý¼àÏ>àO»ˆ\Ý?ïß!D`±?€Øír['ü?po?]Ϩ?€Øír['þ?ïçDöÒ]î?lâè%vl$?h»	-¢"?lâè%vl7?ïÿûneÛ>Òè*íi{@>æFhŒ|U>Òè*íi'¯3FGL J1258.6-1800@sY_í¦a@FjÍØã\À8•ÜJRÀ;wU·Ây?挆`#M¯@
ÜæöC¿@'eÿ¹3=¿älŸædοæ¦(c©ü¿ä¾²¢v"c¿ê–ón¢AGNfsrqPKS B1256-177?ïø¬Šx‰?Mèß³å"?MM×úÞ?Mèß³å
?ï«4G/ù?ä¨g¾³?…2î´â?ä¨g¾³?ïyuqX)?‰)š¿5È?Ñ\1Ôúî?‰)š¿5È?ïÙJ¿I)Ø?j¡'"3øª?sZ [k¬?j¡'"3ø©3FGL J1258.7-2219@s£¿ø¨ô@DAMå"mÀ8®ºŸ¹À;9&º~ìo?íËùÁS-@Ÿ=⎪þ@¶?Ÿ¨&z¿ã¼²ÕÍø¿äº1"X¿çuJ%NT]¿åB!´ÊfZAGNfsrqPKS 1256-220?ï÷ÿ—Cþ?Ra»y6¾?PÑyô}?Ra»y6Ã?ïp3õ@5	?—0jÕ³ç¾?'ùWù^ã?—0jÕ³ç¾?îä öCJ»?•É—†Xb§?¡½ð›ËTC?•É—†Xb¥?î=þUêç?šAZ@§GÇ?¬ Ê¡Q"?šAZ@§GÇ3FGL J1258.7+5137@^¬Óª7@P]‡ qäÀ:±äþú2À<Й
'¡¿þz5
(¯@
¯¼{F@E$¿ÒéG¿¾²lƟ-¥¿æ1±3ÐMF¿æPöñ5Õ¿Æuyv/ÿoAGNbcuNVSS J125825+514225?ïÛÜùqc?†\… õu›?rƒqÇNs?†\… õuœ?ïÕçÙÖ?'ÓÔ'Âu$?u@?'ÓÔ'Âu"?íFI÷?§ÈV±ì?³•Í·PG?§ÈV±é?ïÿª•,]?
d-¼à¬Ý?Z´úh×w?
d-¼à¬ý3FGL J1259.0-2310@swß (@CÓÒòäÀ9·ŸŒ¨À;€Kµàø?äôÑp@§ԖoÄ@:‰à>¿¿Ö€ºÈñÔw¿èS$Ê\&"¿µük­Ålþ¿ãM—"þ÷AGNbcuPKS B1256-229?ïÀj¿Áa?°Ÿho?Êþ O^?°Ÿhp?ï¥Õ'cs?¡P±´|} ?«EO³'?¡P±´|} ?ïw_Hß?"å滉tA?1ä	?"å滉tB?í¿ÿ ö›\?§HÔ*³;?²øK%?§HÔ*³;3FGL J1259.8-3749@s/hی@9$;I'À9¢Ö(–!?À;ŸÛÔ§Œ¡?ÙfJ`»@où¡A-È@îø 7­ì¿ê	‰…i%¿ßÔ«±|ÂÒ¿á&ŒÓ|X/¿Ý†ª,þ'AGNbcuNVSS J125949-374856?ïåÓ¬f0ð?o¿†2'«?j,S™ÏÔ?o¿†2'±?ï9áÜ_ö?¤yXƒ~0%?ŸXÃÄtU?¤yXƒ~0%?î 4¨»S,?¨òxeŸ?¥üµtJÍ3?¨òxe ?ì¡_¼
Ê?©œLa!¶€?¼õ©º?©œLa!¶€3FGL J1300.2+1416@s‡‹À]RÁ@S?ßеÀ9L#Ü~¸À;®d¾£?ÞXìd[Ž
@Œ+·ü1@×:€.Ž‰¿ê+°#"5¿ê©ó~'W0¿äïÉíÛvo¿ïùé÷¢AGNfsrqOW 197?ïý!âT—¤?9­ê4Êè?6ðí[BÞ?9­ê4Ë
?î°>‹-‡?¯aĨï/?¤üOý'‡?¯aĨï/?ïkˆ¥à§á?ò3¤®(a?'ŽëCëÎ?ò3¤®(c?ë{÷›*?±°§ùd?Â!"«Uú?±°§ùd3FGL J1301.6+0832@smD@lÚ@QÐGßþùÀ9D`Þg)À;¨âøˆ<z?î…У_ÚË@
ÙRl3"è@@dÊ¿àWe¿äºH«ÿ4¿æE3w•|˜¿ïÿïʆT PSRPSRPSR J1301+0833?é¦gLŠè€?Çis#`ªU?ÉfbÍÔ]ý?Çis#`ªU?Òÿ(Ìú?ÖaSp©'?æ€k™ý'ö?ÖaSp©'?âu<âµñˆ?¶wV´	8E?Û†:"í?¶wV´	8E?®²íŽôÉC? iëhâG?îÑ'³l? iëhâG3FGL J1302.3-3259@s;?¦Þü@=ÓÝÿú÷ƒÀ94¹šûÀ;'h§‰Fe?ý7ùÁw"@
vêªÙ2?÷…«'	?ïúŠˆÏr¿×Ð.½§¿âwõq©¿í`ö0ã PSRPSRPSR J1302-3258?b¤"2¶?,ºkSRÖ?ïíñþ[{Ï?,ºkSRÖ?wæ̺?‡"?‹4mЮ4Z?ïÐ2f‹€ñ?‹4mЮ4Z?¡
S!$?™ð,'>n?îï*Íí¾ð?™ð,'>k?|ñ"cú‹?nž`ÀÝA?ïÆ÷9Ö?nž`ÀÝA3FGL J1302.6+5748@]ÿò¾ÎÝH@M \ßÔçNÀ:…6ÍòfºÀ<$y'¼U†¿ª±›aþtP@;*Å{u@-_§°^¿ê¡:fпæÍ»
hÊÖ¿ÓØb<`-'¿Üº¯6*èAGNbcuTXS 1300+580?ïùX{Fë?t2[^‰æ¨?JŸ–äTæ?t2[^‰æ¨?ï°­éßÜ?'¤Æ×j¥?ƒÔ…ˆÿN?'¤Æ×j¥?îýCZ¸hh?¢!JÓÇF? +ÊTyy|?¢!JÓÇD?ïå敦W›?bÖ î1DL?jjY¨cA?bÖ î1DJ3FGL J1303.0-6312e@sÃ{á"¿Öâ:""•À8'£¥AÀ:NU\Rç.¿Ù™bìc@Æ_Ȓ€v?úDå)?ïú-Ç©­¿åhlÐ㳿â1¢4rÎ?Á!™h§^OTHERPWNHESS J1303-631?ëÿ‡‹Wî?¼mÖLa?ÀáÒ£¨P?¼mÖLa?ëŒl>â?Ð\7û]á?ÃñÎO¿t?Ð\7û]á?éù_'†ü?±±ïo³kc?ȃcáä?±±ïo³kc?ïò;_Ï?e"Ûm"ù?[ù‰AÞa?e"Ûm"ù3FGL J1303.0+2435@uՍ@$³>@U—‹àôÀ8‰ñ…é¹À;m˜«]|?ëÒb?‡¡Â@»V†''@r±¿€3¿ØÁ'H¹Ï'¿âú¦ôÃXQ¿ãڔßÜ°+¿äNÆýTÿâAGNbllMG2 J130304+2434?ïó[y|û?hF
åì?YIÁ
q?hF
åì?ïÙ'黓Þ?'¤=¥è•?sl"6Y?'¤=¥è–?î¾æÇÿ3ù?›B¤ñ¡ö?¤"€ÀZ?›B¤ñ¡ò?ï÷btgÀì?MÐëÎ\çÎ?Q;0~)T?MÐëÎ\çÐ3FGL J1303.7-4619@s~KZ@0ñ'lÀ9t.¦¸§À;ŒËÔHµ¿çƒÑ¡¦a@+‡ø[Ç@]à
Ü¿çhc'\ʗ¿ãÁöçÊÌd¿çfå\š=¿ç@>"iPAGNfsrqPMN J1303-4621?ïî—åµô?a\ŒýÕZé?ah=J
U?a\ŒýÕZì?ïÔ÷€?òFëPi?u"?ÿõû±?òFëPl?ïEa9oǙ?~Ýf_š?—SØÒä?~Ýf_—?ïë±hЫV?a܏"ÖB?dN—/T¨‹?a܏"ÖG3FGL J1304.2-2411@s*³ S\ž@CJà€øÀ9¤0íCÀ;yIoH?ê¸-ô¸Å@¶ì²Eb
?ÿPò@¤µ×?ÕPHÌfdR¿ØIµ‹g§¯¿âAÇÝÇp¿ÚØ/ßõ&;AGNbcuPMN J1304-2412?ï³úW	U?€ö>w,?ƒj=¸+?€ö>w-?ï3Æòÿõ/?ž°µ*d?™‡! Z(?ž°µ*d?î;éáÖû?ž\¹¸¿?¬AaâN?ž\¹¸¿?ëæ ¨¯øö?©QÍ£?Àe}]@#?©QÍ£3FGL J1304.3-5535@s^¿¨÷Û@ö© JMVÀ9xþï^ÈÀ;-QîÊN?õC5Ú£@'Øì?Ùµ@'/ÀbY¿ßðë(ò+¿ì¤¯ÿ;_¿çJÒ6C3¿ÝßQ‹Û7kAGNbcuPMN J1303-5540?ìÚ¼äÛ׀?·5"/ôµ{?¹*Ù!Cù?·5"/ôµ{?ê½ù½'é¸?ÐèþÅ¥×?Å	´Y?ÐèþÅ¥×?çW±Ä)›y?²Þ6c!8?ÑPœw¬É?²Þ6c!9?ׇouTà?Âè€[øÌ?ä<H{ÅU?Âè€[øÌ3FGL J1304.3-4353@s[ߏG0@2逾À8D7guZÀ:Úá& %9?ä³i0Ü@D‹çTbƒ?þ…ÜiM¿àlõÈÞE¿Ù1Ídn¶ä¿ØÕN\j C¿à'Í2|AGNbll1RXS J130421.2-435308?ïû˜De[9?I–…¤Ç?Ažîj"?I–…¤Ï?ïÀœ43
Ë?ƒ…à¾6}?±åæzšý?ƒ…à¾6|?ï¡;EºG*?†h¼+›j?‡±.'n5L?†h¼+›g?ïÌRàh?¨M¦·ûf?œÆu£ý
?¨M¦·ûg3FGL J1304.8-0338@sWÿŽÀù@M†ÿ ^¯¹À:ažõ!À;ʆ`ñ˜¿Ì$Ǟ±ÿ@1mÇXÅ@>€ vÿéìÝîœe¿Û©VÉmû9¿çñÊ8%"ì¿ÊÔ¾!¨
AGNfsrqPKS 1302-035?ïõ‹ºË4?aN ÊÞO?Tè‹Äi˜/?aN ÊÞN?ïÅϨòô?‡X£àa?}+·†…'?‡X£àa?îó<ç³w?˜Xƒ=ñ? Ì1"ȏ?˜Xƒ=î?ïø®	©Zí?HOµ†?MGÙZ"MÙ?HOµ†3FGL J1304.9-2109@s2"@lÚ@DÍ0úŒ#À:7Ϗõ«éÀ;™S ' ?ќ®Ñ(@¥í¤ܘ@.ÜÿÊÐô?ïÚbð÷4¼¿ê.f›Ñ"l¿×¼<a/Dç¿æ2rgâ¤AGNbcuPKS B1302-208?ïþm%'sß?0y̤ù
Ö?)-­ˆÂä?0y̤ù
Ò?zf§®?¬,ßkx˜?¦Å¨Y•…?¬,ßkx˜?ïjAœ.S?‹~øCyx?'·Ìz.t?‹~øCyx?ì¿,à§gÃ?«ï]Fí4?º˜úÄÁì?«ï]Fí53FGL J1305.4-4926@srÿÑÜ×@*¿?>Ú0cÀ9 ×{|xÀ;jmH÷Q¿âU©´]®÷@)ê'/—ó@j`_'5¿å²À²W¿çXÞ=¿âÆì]¶¿o¿ãõç]qËOTHERsbgNGC 4945?ïøy9ôr?Mº+X—?N‹.9Ù?Mº+X¦?ïÃØ#Á¹F?"y[²Ö¿?~î#\÷?"y[²Ö¿?îþqý³-d?–‡N»¼.d? à$Í)¿?–‡N»¼.d?ïÅê95×?w'¦?}
ãe{È?w'§3FGL J1305.5+7854@^"‡aˆ±@Cæ@;YrÀ:	!0Ò/ãÀ<¥šXÜ:¿ï¶ö˜'ö|@
Û'òã6ò@ߚ¯Ä¿à¤kTôÏ¿å€ÚUÌ¿æ+ö8+¬¿ã™{!ð{åAGNbllS5 1304+79?íWqqiGG?À]*×y?µDttµÅÎ?À]*×y?ïÔI¼r?ª'h³&?ž<åvÈqç?ª'h³'?쇁'TÅ?±yh9¢ey?»ÃöÅY׫?±yh9¢ex?ïÇôt˜œç?zŽX=?|ų±Œ?zŽXA3FGL J1305.7-6241@s	&ÿ}ú?ÁúŠ ,…ÅÀ80·omv%À:E\jd!é?㳐Núu@r¤@;¯@΂ÿú Ã?ïüÙ9™m¿âó^œm‰p¿ßÊ'Áe¤¿æÃx;%OTHERsnrKes 17?è€ù"1T?ʹ=nEâÌ?Íü¯;Ž²?ʹ=nEâÌ?âIñÀmþ?×ßÆ£†Ò?Ûlð$?×ßÆ£†Ò?æAZ-tž?»O1Ê6B¿?Ó}Jå¥Ã?»O1Ê6BÀ?ëX-–€Áv?·ÞŽÑBÚ¯?ŸI¥üú)?·ÞŽÑBÚ®3FGL J1306.8-2146@s:É?¯Bx@Dyá`xÀ:I9¸ˆr*À;•"ô έ?Ô¸>Ã5@¨ÇÄû@@,Qy‡Ö¿æùx`}²ø¿Ü÷q¾*À¿á¿°ÁË´@¿åÌÔ^çl
AGNbcuPKS 1304-215?ïߕŒV°*?o&B%d¦?p59Ô§ë&?o&B%d¦?îl¨¡	€?­™BY4»?©5uïnè?­™BY4½?ï?3!Ùã?'\»qAU™?˜›ÞdÞ?'\»qAU›?ìûó«*=?«5µ£sä?¿ð b¦®"?«5µ£så3FGL J1307.6-4300@s!] l‡@3Ň?úÁÓÀ8yÜ>Y×ãÀ:øž0Ø ¿Ö3ãVüæñ@A×*É­3?ýf	AGH¿ÄNñTÁx¿áæF!'9¿Óôõ~"¿×´]a§\AGNbcu1RXS J130737.8-425940?ïöܜªXÀ?Q>E]±¿M?RFÆ«N'Á?Q>E]±¿=?ïÔ'D?~Zæ³´®?uò·t]öI?~Zæ³´°?ïœå[l^?†ß‡{*VÈ?ˆÆ©$ùèr?†ß‡{*VÈ?ïçës–há?g¤óKŠž?hŒi—;?g¤óKŠš3FGL J1308.1-6707@sþÀ//˜À4›ÀzÀ8kË^7üÀ;ȯ0ړ¿çÒ:"T'@"ÿŸ‡ð@™ÿ…Vl¿ä…H=JR"¿ç_ωÿ¿æf  Øxä¿år›ÞàæAGNbcuPKS 1304-668?ïø¦?uËV?Ró {1‰†?Mg(Ò¦Ð?Ró {1‰"?ïGìõüþ
?«ßÓ]Ö.ö?—a@`>º?«ßÓ]Ö.õ?îø<rþïÆ?—çPZ§y? |8А?—çPZ§x?ïýT¾ÇE|?5¶‡Ÿ¢?5Z	ÅÔ*'?5¶‡Ÿ¢ø3FGL J1308.7+3545@Y8¬À½ÊÑ@T'Zà f¨À9®"ƒ‡ß]À;߅¨K
E?×ôNšÜ~Š@zŠô[é@ÚD€"
¿âŸ ®1'¿ä°ýëü¿äNdíÈùa¿ì´@d|´åAGNfsrq5C 12.291?ï÷ó¨éÆr?QPueÿ°¨?P®,s?QPueÿ°¡?ïˆôg?†a—R¶è?z<…Ì|ÀK?†a—R¶ç?îτûÔ7Ã?™BoÁÅ¥(?£°B¼ƒÂ?™BoÁÅ¥'?ïèo,ö%h?c#ž©ã§à?gÓ	ژ?c#ž©ã§ç3FGL J1309.3+4304@[Έ~¿"À@Ri*ùš‹À8¤D¡À›À;Cä1m`V¿÷¥Ýað_ú@±«3J?þù_Js¿äBûxdsP¿Ù|ÙW¿׾íñµn¿ä ËR+úbAGNbllB3 1307+433?ïày˜Å0D?¨À°mÃ?o†g:Ϻ!?¨À°mÃ?ïÁä9nš?IÒØu<æ?
ãH¿2Æ?IÒØu<å?¹Ñ$?Š³7Ùa`?ŽÕ?Q‹·?Š³7Ùa]?ïùˆ³´«Õ?WɊO‰¼µ?IÝ1-P­µ?WɊO‰¼¾3FGL J1309.5+1154@söÍÀÓg@RŒ "µ7À9¿þÆDÀ;®ÛÇ4Ý?ߌð;Å[@¶EF0@%6€o§?î2†wÓÌ¿äp®·h•¿Ô
Û«X*¿ë®Ž
ÒÚAGNbll4C +12.46?ïC?£ Œâø_†?žŸ]nW'?£ Œâø_‡?ìo¬ ?Ä0ï-'`?»‡ÜƒzŸ?Ä0ï-'`?êyDh2ª8?°×®%¡?Æî_5W$?°×®%¡?ê×ÅEâÚ§?³¢F"Nzß?Ä êèt•b?³¢F"Nzß3FGL J1310.2-1159@sc@@IOjNÚYÀ:4Þ]	À;§£3vO?Á"Ç<6‰v@
Ãvõ׈?üÂÀ¿xPt¿èãeJ\š‹¿Ð|û3ßοæÒYÏ:w?Ѥ\&'²AGNbllTXS 1307-117?ï&>¬MÑd?Ÿ¡ê®-ý?›8*vEÓz?Ÿ¡ê®-ü?ïT_ë¹ÂÌ?­™éMùN'?•tˆÇ¦–?­™éMùN?î]€mjúC?¡[0¨&Þ?ª'ù)P[Ê?¡[0¨&Þ?ﱍ'Þd?'ô1'åb?ƒœ¶~&ä?'ô1'åb3FGL J1310.6+2446@­öàF§.@UFãåîÀ:¯3‡	WÀ;à_?³UX²Â·*@
U¡¶ž@jÿ¨AR¿è´ Â>¿é)"R#J¿Ý)nÛ¢J¿é¸ÞصZ¸AGNbcuMG2 J131037+2447?ïý
Ê_WË?: 5ŽI?7©­A¦ë?: 5Ž?ïA_yF-?¥WY fÉ?—Þ"×:s?¥WY fÊ?î­RHrŒ? 'uy[šp?¥*Ûx×?Ú? 'uy[šo?î8"_™%h?¥kNgvï?¬wºm©y?¥kNgvï3FGL J1310.6+3222@Ugáßîè@TÓ¤à¹)À8éqHA¸À;2ªýo?ô6°x®<"@IG¨¶)@8ž_&+8¿âr<Í)®¿ã`=þúW±¿äjg="¿èºùŽ‡ÿAGNfsrqOP 313?ïå"r oø?xÖ
ˆ?jk_?xÖ
‡?ïÓËiÛ«…?"Ätti?vK*=Ã?"Ätti?íçXߥô?¡»ð¹Z¦f?°Å9Ð_Ð?¡»ð¹Z¦e?ïð«|P$i?Zw¸ç̦˜?^©_·,J?Zw¸ç̦'3FGL J1310.7+5515@]I^_0çÿ@NÓ# 8ÜÀ:V÷~0ˆÀ<
 Òrÿ¿ó&—ºo@¿ênô)ˆ@7»Ñ+¬¿èi>Tpè¿é¯"4LZC¿åjY­"¿ÖÅZ¡¥ñ[AGNfsrqTXS 1308+554?ïÿ_¡-!A?!gȯ;§?Ú[×ÇI?!gȯ;¾?ïω•žÁs?†è~Š6Ž?x;50ŸFÑ?†è~Š6Ž?ï€êÒFKÁ?='¨òõ«?ÅKnm´?='¨òõ«?ïÿ'zí«Ò?F>þ'?aD•;‰?F>þÉ3FGL J1311.0+0036@sB¡ Ï@Oˆ×ÀEÕÍÀ:¦.fDØwÀ;­À8iÓÙ?›j)?@vwY}Ë?ø¹€C‡>?î7¡Zî¿Ð
µ|Æq‹¿îw}»þ¯"?í0ÿ1#
¡AGNbllRX J1311.1+0035?îÎýyaVÖ?¥Ü®lœ—X?£(i꒟?¥Ü®lœ—X?ïUÙ²¾@?³(Ñ@ÞiW?•Dɨ<wç?³(Ñ@ÞiV?éÊÞ?²\žÝý>?˯äԇÓÅ?²\žÝý>?íp'šæÔ5?¼'èÛ^è?´{k(É^S?¼'èÛ^ç3FGL J1311.8-3430@s;0À&Ì@<.Bßx üÀ7vßY—KÀ:þ™‰©aŽ@ŸêŸñw|@ª1ëàcX@Yèb|¿ß\-WÑù¿â`ЛŸ"l¿æ!±U¢ô·¿ì?@]EÞåPSRPSRLAT PSR J1311-3430?më3¢Ðkå?iŠ.…	Ÿ?ïâÌ]/"?iŠ.…	Ÿ?»k(°?'Ø>1t
þ?ïÀ‰)é¯Ù?'Ø>1t
þ?¯ýY²??¡ðÊC,ª?î*dßÏM?¡ðÊC,ª?bhìÎtX?_·š›J:c?ïí—ï1Œ?_·š›J:d3FGL J1312.5-2155@sVŸ¶M@DV}€^_1À8¢kË*5^À;9ÜO σ?ñlP5L"@Ž©-
z,@™#@¡Û²¿Ý©á§òš3¿ÝŸ^Ï('¿á¯ýã¿ç:ˆ»ê–%AGNbllPKS 1309-216?ìÆ|"ǎ?¶˜©ù$—Û?¹ÌféÍ?¶˜©ù$—Û?äc·û'çc?ÊÖf?×8Ü1:?ÊÖf?èes ±s|?´l¹.Ù?Îj1}:2?´l¹.Ù?ÛS¯Lü¨?«Ø#gHL?âV(Yù«?«Ø#gHL3FGL J1312.7+4828@\We^(ªC@QiÿãzŽÀ7Ägˆ¥UÀ;ýG¾Ûs?ð¾Eہpƒ@ lf*"Š@Y?ñ½ß¿Þ.3>ƺ9¿ãØ:Ö.#¿áNÊwvÈο䝞ö>¤ðAGNagnGB 1310+487?ïÿ5µì?#Ԓ"ØÇ?YI^º¢?#Ԓ"ÙD?ïج`c±?'½ûLå@?s©øOÎ'"?'½ûLå@?ïqÄòüŽ›?"›G¬
?'Ça n,–?"›G¬
?ïÿÿlîà€>¢¤®(Gb.>'b#ïØ¥>¢¤®(FÿL3FGL J1312.7+0051@s­›6†¥@Ožm?ž{À8Óî{s=åÀ;‰Oçžà*?ÿˆ¦½@°z‰^
'@öp
Y.ð¿Þ¤ÍÔJð¿Úï}XgÂ~¿ç¢o-Ô¿í9"Paí0PSRPSRPSR J1312+0051?S§(7Ç3´?Q²S]¿?ïö,käe?Q²S]¿?³Ñ×[M.{?È*Í£ÇÄ?í…Å–Z2?È*Í£ÇÄ?»=Ó Xo'?±žœòë‹?ì˜E›ôò
?±žœòë‹?pG(GÒ;D?a×ã%_^z?ïßq¯p[ˆ?a×ã%_^z3FGL J1312.7-2349@sS6@c^@Cdó=<¡À9£úoFÍÀ;gXv¹šÁ¿î6÷'`¹v@tÎ0?üÒX_g™—¿éS''Õ¿à"ú Å‡ß¿à1oóœ´?²¯'ÓÉ/AGNbcuNVSS J131248-235046?ïþT@ÙG?('ÅGT'?*»òk	Í?('ÅGT?ï̹¢ä+*?"yËõ›;?y£.êk¡?"yËõ›;?ïº|`fL6?€â.^w¿Â?`çælòÓ?€â.^w¿¾?ïÿM¬Iz?= úQ›"?N
vэ?= úQ›€3FGL J1312.8-0424@s'#ÿï9@Mé_ªŠƒÀ8ü2Q‹ãÎÀ;"ˆTÍ·®?ßý»Õ"Ù@Ø´ž­ªž@åÏ_¤*l¿âvÂé—U¿çRhÉþÅ¿ç Q¾+¿äâ!…U<AGNfsrqPKS B1310-041?ïÿcô¯?#¤ªfê;?žjb?#¤ªfê?ïÏé"T?…pwiÙ
?x6UüôÃ?…pwiÙ
?ﱐ9'ç?¹ÅèôF?ƒ¿›ñ›†I?¹Åèô>?ïþÓj¾J? 4	7Ï?"ÉT[X? 4	7q3FGL J1314.7-4237@s7üÀz®ó@4	›€#¦ÎÀ:Edè·äÞÀ;Ø
°÷?Î=ÊïZžæ@u!àO‹"@¨_–¾s¿çš»…Û)e¿Ý‰áT2 (¿êß¹Yí¿ÙaÆ¡´AGNbcuMS 13121-4221?ïT¼µI?LØc—?•}iVØ?LØc—?ï°[•‰?'½'z
?ƒþ¾i–?'½'z?îrÖÒâK?¥¬.Û?¯ҒÑÛA?¥¬.Û ?îÜp³†íL?–öý'?¢8ôǑ+9?–öý'3FGL J1314.8+2349@½Ðÿ·ZË@Tñ9èîlÀ8ß½×fƒÃÀ;ltK+w}?å±n Ø¹P@à÷Gʙí@b,?¤Ø¿Ññ¨Ys¿ß¥!¢'¹¿áÕЪä¿á§ÊlÓÆoAGNbllTXS 1312+240?ï CYÈÌè?œ'÷o¶[*?›÷"Ææc'?œ'÷o¶[*?í*Rüß?ÀëÆS¡9š?¶¯-h`ÿ?ÀëÆS¡9š?îȵë?Ÿ3éŌÂ?®Xt¡O?Ÿ3éŌÂ?ä?¡-CØ?À@,.I™?׀½¥xOÌ?À@,.I™3FGL J1315.1-5329@s(`ÐÕ@"p'`@3À8Π°P%À;7€ KÏâ?ú¤Q›©@C¼«Âf@}KCuJ°¿áS-ë[êH¿æî¸É÷¹¿ê£Ó€‰ìí¿ïþ[2*ʄAGNbcuPMN J1315-5334?ïœ ó»/–?‹MP'ùé?ˆ÷Ã4A?‹MP'ùê?êaaB‰?̀'ú3e?Æzz÷¯'Ú?̀'ú3e?ëÚgÈÌä{?«£@"+?À–`ÜÌn?«£@",?âƒ4	®?¼½wّÎ?Úù—íÔ£Ä?¼½wّÎ3FGL J1315.4+1130@t?'Àa"@RYg 5)­À:'ýýûCÀ;×íÂæ™ý¿ÃªM›œÝ@+A҈M—?ÿdï`u‹¿íYo7¿áXwŒÒ½¿ßW.e3?Á?jƒ×e'AGNbcu1RXS J131531.9+113327?ïýw×î×-?D僧nˆ?4A@‰F£¸?D僧n'?ïÔÉS»ß?ƒä<ãFä4?uüV"1?ƒä<ãFä5?䙖«?ˆâ®FtEô?Š˜ÆٚUB?ˆâ®FtEû?ïöù–ÙsŠ?R²ðŸW‰˜?RÒMë"?R²ðŸW‰¦3FGL J1316.0-3338@sL^`=Wy@<ñÁ'°—À8I[	T=À;6jEî÷š?ã˜ÂÁÜö@Bv2aQ)@"ül—¿à*¶Fšæm¿åuµÃ_ªy¿å
H@5¥(¿æîÅ%ñAGNfsrqPKS 1313-333?ïýŠôFÞ?2>U&¶5j?3¨_UÉ?2>U&¶5[?ïÓÜ	M*=?W$bT!h?vûYjád?W$bT!i?ï#0DÚÃ?'¸*e˜?›™÷d½Gt?'¸*e˜?ïþ'Aë?$êyûpÀ?&îáN•Ø?$êyûpÀ|3FGL J1317.8+3429@UÀ4 -œñ@T-€/eHÀ:7m¾I|KÀ;ñò';×?ÊLNöeÕû@›ôgÆc@«Jàxü¿å(­Q÷x¿èYV¥ÿª¿á_«ÀHì¿ïÿ¸JÅÝ+AGNfsrqS4 1315+34?ïÿ"©Åá†?ǝVd?
Վ‡ž«X?ǝVc"?ï'÷Uœª—?™ú+æ'ÐO?B*˜ÕZz?™ú+æ'ÐQ?ï´d7#E`?'ŒÑ*kÚ?'æò7.¨?'ŒÑ*kÓ?ï°Æ ë<?"ñÔoÐf?ž‰ç+â˜w?"ñÔoÐe3FGL J1318.7-1232@s"¿Ÿ‡ð$@HãÓ %¤ÕÀ9³ '²ÌÀ;¨—¤¹¿ï'Ž>;@™íÎ à@ǹà`þH¿äkB	K‹¿ä¼0LÎ嬿æÃq¦­Ì¿áÓÞTð®eAGNbcuPMN J1318-1235?ïý¢w!Õ?9j€øo–ù?2ìFñWü?9j€øo—
?ï¹þ"
ô‹?‹=˜è;±?€w}BÝK?‹=˜è;±?ï¦ñêàZ?"öÑÅو?†C…Gúéw?"öÑÅي?ïúÀLM¹?B¶ýiœÅ?DþÎËù¶?B¶ýiœÅ,3FGL J1319.3+1402@t¬–ÿÁß@RØû_ò®ßÀ:Նjè¬&À;ýŌf«0?ãPŒ~^ú@H§Ž¤É?ý؜žÜ¤†¿é•Øa€x‹¿Ùï38'—¿ÙDh(¢$q¿Õ¤ýä$Š×AGNbllRX J1319.4+1405?ïâ¾n•*K?q.{ô?mA'jÕµÛ?q.{ô?ï(þ£±^ó?«	ŸiÇT?šà+‰Ô!ª?«	ŸiÇT?ï ò)iÓ?'#´
†ÿ?›áºÒş1?'#´
†?ë~"'Š@a?¶6Óoÿ?ÂuõÖþ~?¶6Óoÿ3FGL J1319.6+7759@^CE€<ÑB@Cƒq_¾¬yÀ:2ÂfA}yÀ;äÚÔÍLO¿‰9	`üÅ
@—½Clç4?ü'_øc)¿äé»Qп×w3£E"à¿å²R^OI?²×œù9VAGNbcuNVSS J131921+775823?ïÍ{l+Ÿ½?"Óp­¶Y?yBIê0!Ê?"Óp­¶V?ïÇÄúm?""õ3«´Á?|}ñ'ÉÚ?""õ3«´Á?ïgÌ1G†?–pã£å?Sy×Q?–pã£ä?ïÚÛæ!p6?nîïóãø?r'ïGä¡?nîïóãÿ3FGL J1321.0+2215@vj¿ß~€9@TlŸëWÒÀ8ÆÄŸäÀ;zŠPPzl?Óô½¨RÖ"@YÌ­ÃJ@_ÄŠŠ¿ã–¤'çã¿æݳ*u…¤¿âÐ1ú+³@¿êïgMä[×AGNfsrqTXS 1318+225?ïþê2R?$n²ìËúÐ?!^ÿ¼Ú×:?$n²ìËû	?ï˄ä]MÇ?‡O ¯L
?z=ÑYÌ?‡O ¯L
?ï"bŒå,É?‡Ø.¥ˆV?‹'\Æ´Î?‡Ø.¥ˆT?ïß+϶´?h3o;¢?pj$¥ýÂ?h3o;¢3FGL J1321.7+8312@^vÖÿ´@@íÛ L¦¢À9ˆœ×;»˜À;å#ôÑΔ¿úŸ-èE¤$@¿:òð"@"ÿï¿çÿÕJF
¿å[ËÙæC¿ä-"XÐâ¿ìຍZ)AGNfsrqS5 1322+83?ïõŽWÍ!ˆ?XeG	_­?TãPe¼ïY?XeG	_­?ïÖ¿Ry"J?•>HÃf?t VÃnÛp?•>HÃf?ïwP>Y¯?D¨am{?'ø=Ê"?D¨am{ ?ïÿÓ¾©p?c›ïW">ö «pHh®?c›ïW"'3FGL J1322.3+0839@t_._ú;›@Qˆ¹`~TÀ9êk#d‰À;ȓ6©	y¿í0ÇA-Øç@5KÈÊà@D_ÖT`¿åªü°•3®¿ææ*cMO¿Ì-Ìnâ¿ïù_'aÁçAGNbcuNVSS J132210+084231?ïõm )?u$'@ÛVí?U%¿­Ðä
?u$'@ÛVë?ïË´4Uœ?ˆåƒëN?z%å÷Õ2M?ˆåƒëN?îA«™–ú?£› 'Í·?®«åFf]?£› 'Í·?ïüF˜"—¸?Ac։kr?=Ë;cB3?Ac։kr‰3FGL J1322.6-1619@s›§ÿyÈ@FòÖàL'À:…zþ£ßÀ;´°t§qÉ¿öÁÊóƒÅÈ@
my=¿Î@Ùö X:)¿ãØ_'.¿å‹öº±í¿ä2Äߝ׿äuø»Ï5AGNbcuPMN J1322-1617?ïúd4aÝ
?I§!¸ÝÆ?Fo.x‹Ø[?I§!¸Ý×?ï¢Ã¶ñ›]?'§hĎÑ?‡OC™(ô?'§hĎÑ?ïMUÍ?™ó—Êr(?–NNF\u?™ó—Êr'?ïøªñÁ_a?P·3-³m?MT8ú'}?P·3-³j3FGL J1322.8-0938@s»î²Ñ@J9JÞ™À9ò#žjºÀ;—ÿ'E7?ßÕs順â@½×Zob9@	Ÿ#•¿ç˨÷ý¿åäÁ ØMñ¿ìböuÎÊd¿æ6É5œ!½AGNfsrqPKS B1319-093?ïþP2h2û?*BMa‡?*üÙ|ÐBà?*BMad?ﮑ×Ë^?Ž
"Nâ.'?"[Š>(Š?Ž
"Nâ."?ï'ËÎú?ƒârÈe8"?‹M<|¬?ƒârÈe8'?ïÎjÃW?räåˆñÅ?xøJýTÖ?räåˆñÈ3FGL J1322.9+0435@t,@FA-@PìŸÐë?À:_nÔÉñPÀ;³gþìډ?é
Ƨ™·w@
¡×ŒÄI?ûÕP~ó{¿ïÿɯ"‹E?ïúK"	¸¿Âá‡é\¿7¿áfŸ*ÀAGNbllRBS 1257?ï꺢ÿPf?cã€ìÉs?eE]¯™N?cã€ìÉs?î:_KEA—?´Ø(d&öÉ?¬ZK«æŠ?´Ø(d&öÊ?ï&B¨ŽFÈ?Žx¼ªlžž?›7ªî7&ß?Žx¼ªlž›?ê8Î_0Rx?ºÍLÏyJí?Çƃ>¶?ºÍLÏyJí3FGL J1323.0+2942@Kš¿¨!@T¦$`1˜ÿÀ9Τ…À;"Å@'H¿ßÄßv%T@.ëí¤^@)KßÒc¿á~ÚxSp7¿àQs.ZË¿å)zûÒQz¿Ù0àí¥AGNbcu4C +29.48?ï{ùŸª7"?"65Œ4?€Ì
¹–?"65Œ4?ïB:m€&4?«†­0ª?—¸²Oû9'?«†­0«?íP*4››?¥»-Of?µ~®[#+?¥»-Og?ïA€0\'?•\ú)F,3?—Ïùôm½?•\ú)F,33FGL J1323.9+1405@tì¿ðEx@RºÅ_ñ_À:1Sϊí.À;Ñ#2ý?ß;¢9¦@¡Û1"x@›·1Ô?ïÿ"77y¿¿Ý^?ðt¶z¿ãA?ØTŒÂ¿Üã?AGNbllRX J1323.9+1406?ïìbåÿĊ?j	8N—p?c;vä?j	8N—u?ïuJ)×? ATìŽæË?'Vºß? ATìŽæÊ?îÊ°€¹:¯?™¡lTÌbó?£T÷ôlU?™¡lTÌbô?í‰ÿq1·?§I†DÍU(?³°vr@?§I†DÍU(3FGL J1324.0-4330e@sR°€0<@2ú!€ƒHÀ7¯¦Ç…òÀ:4>ª_º{?Ó°ÙpcI@O92¦›`@94¿zSٿ僢k80¿ésr࿕¿ç4ú|»¿çRÌÒ<^'AGNRDGCen A Lobes?îi‹ia?²Y«=õì?©gInÆùè?²Y«=õì?ïъþøÂ?'½¯I-ë`?w:€ƒž?7?'½¯I-ë`?ç½Yåëw®?¶ÛÊFPœ¯?ЅL4)¥?¶ÛÊFPœ¯?ï¡ÿ™ôc?'Ò#E®?‡€»'ç\?'Ò#E®3FGL J1325.4-4301@sXA?ÐÐh@3gßÿ¯x(À7oB¸âÀ:ç|8_ÂÞ?ê1M*Þ®@U8âtª@Ÿ¹<:ï¿è:ªmHпèãÊÀŒ¿åÀæøД`¿âwÄËT/`AGNRDGCen A Core?ï
*ØQp?§ØP¤@?žº¤ðÒ
?§ØP¤@?ç5?¹ÎF?Ð*ªh)?ѕ€Œàct?Ð*ªh)?è1‡–í?´ðä.yþ?ϋ9㱤H?´ðä.yþ?ØI»¬e?Á ³Á6©?ãÛp"p)Î?Á ³Á6©3FGL J1326.1+2931@J8ïÝëÙ@TڿԖÆÀ:²/ÍM%MÀ;ѝx]¿ô
%\ÛÎ@…"'|Ç@Ž@?`=-¿Ú˜D¦3l$¿é¿F™cá¿ç‹ø&Ì{?ÊWÍ.Ïÿ»AGNbllTXS 1323+298?ïþ54eö?-4ÝõÊ»?,¬¿y ?-4ÝõÊ»?ïÓÌIÔÌ?†¨Ç‰ÓÃ?vÛ™ò'?†¨Ç‰ÓÃ?îC?+áW~?¢°Û?õ+?«Ì
Aê‡þ?¢°Û?õ+?ïÿœÞŸ¡
?*^@=o?ÈX¼i¿?*^@<"3FGL J1326.6-5256@sDÊ€à@#!Kãö	À8?ŽîDì™À;}\L11?æ%í‰t¢-@•‹$‹Ðƒ@ùÀ›f"¿åȨͿäʳÎ+пä±m7ˆNæ¿è|¬uAGNbllPMN J1326-5256?ïûMÎÊ?CƒèXe
–?C'ÈÇÜØû?CƒèXe
"?ïƆ†Áƒ½?‰Ó2"4æ?|¼¼Ÿ>!t?‰Ó2"4æ?îì?þt|?—cò$ð÷š?¡>L¸U?—cò$ð÷š?ïü\ç8Ê?7µ:䞸?<Æ9·‰?7µ:䞙3FGL J1326.7-4727@sQ§€w‰¤@-÷`¿]xÀ9]5õ…R»À;ZxOœöE?ýèªMñÐ@È?ânÂ?âC`èo?ïþ¤žv¿Ðû÷\ÃOv¿å­Ðrû¿îÂh?"zNOTHERglcOmega Cen?§u®Á
Y-?¬Ÿã)—9?ï*m?¬Ÿã)—9?£ÏkÈ#?½qZw5Ù?îÃ	C~>?½qZw5Ù?¿á¬î‹Öj?±gÖ®h¦½?ìÊb.…3?±gÖ®h¦½?­:´ãóh? 'øƒ«u?î,T¾ÁÀÉ? 'øƒ«u3FGL J1326.8+2211@
o}ÿ_F7@T#kà"êçÀ8¤ðÂuZöÀ;f's"L?õ-wTuM4@"Ëõak€@svënοâî›
²á¿æ¡99mÆ¿è›–ýïܿ璂/‰tLAGNfsrqB2 1324+22?ïûq°õ_û?EۇýÕ}ñ?B9<*€
?EۇýÕ}ê?ïAsŽ"-*?©0À™"¤?—ÑŽ;ºZº?©0À™"¤?ïݽ¬'m?'©Um©èq?œHJo²F?'©Um©ès?ë©çüV?µFÕÁ­?ùXcô«?µFÕÁ­3FGL J1327.9+2524@7·_}>@Th—×5ÜÀ:üײÙ܀À;úé¦Ù¿®É÷G")ï@Æç¨pL?úڒ€Ê÷¿ïÌ»N9Ö?å¹Q
ô¿êlMäF?áªÅK#>ôAGNbllNVSS J132758+252750?ï†Ç¶Qø?š6µŒ5Ó?ŽN'k'B?š6µŒ5Ô?ï¦Ó£ÍF3?—®Þó>?†K®s?—®Þó<?íG¶]T¼?«wÉøiÍ?µÂMZ»?«wÉøiÍ?ï¸Übkd¿?†‰ æS(e?Èçe&Ð*?†‰ æS(c3FGL J1328.5-4728@sVž²gÇ@-Ø->ýkÑÀ9=E†SÀ;2îiՇ¿ò³CÛ[@T¸ëC…f?û0ßÞøH|¿ïëâ§)¥?씪¯Ê8¿Ûù)ßCê2¿"uv'EóˆAGNbcu1WGA J1328.6-4727?ïù®‰[pL?GˆÒãŒ]?IEڒ>Îó?GˆÒãŒz?ïãÐ}Ê,?wã3EëU£?l/'5Óÿ ?wã3EëU£?˜Q¢â?‰hñèTz5?ŒÞYë—GØ?‰hñèTz7?ïþ¢ƒ"¡?,'j®L¨å?%×ÍÕîb?,'j®L¨l3FGL J1328.9-5607@sBÓ@N¤©@nÔ?²ÈjÀ7`>"E]À:ÅÁ:c©?ü©}å‰N@­ègÝßÅ@sÃ²ñ¿áäŒö·Ç¿å¦ìXáÌ¿æòhElN¿ç?¨ñóš8AGNbcuPMN J1329-5608?ï坶Œ9™?iÚ¯y÷è?jbIsÆh?iÚ¯y÷ë?ï©X'(\? â»³?…©ßuøé? â»´?î;ê¾äçL?¡?¼°M&?¬AT±‹$?¡?¼°M'?ïòÖ_hËÆ?\kX«$W?ZSA.hr?\kX«$X3FGL J1330.0-3818@ss?À	oë@7ð#¶eÀ9´8ù€ŠÀ;u±ƒ›*"?äwɘÃc@
Xâe,@>Úà5à7¿éÇúÇÔ7¿é4ÀÜ©Ž¯¿ïÿ	(®Ü¿æäy<_Š]AGNfsrqTol 1326-379?ï¿\ÓÀ<?…¾V4âº?€(Ë=Ïðô?…¾V4â»?èwê¶`´?х4º$?Î# U&}1?х4º$	?ìV"æcŠ?ª7C«ð?½K`Ìã¯r?ª7C«ð?гq(ö'2?ÀóÞ‹àP?ç¦Gk"¶ç?ÀóÞ‹àP3FGL J1330.0+4437@YeÊâ°@Q·: þ¡À:V'šx¼ªÀ<¯ÑêC?Þݳ¹DHž@rѹp¤ƒ@4¬¥Q´¿áþØöPÔ¯¿Ð×ͫοá‡À[ØÌ¿ã@	ʦyHAGNbll1RXS J133021.4+444117?ï½6î«{«?ŠNÚíë˕?€²DU!Z?ŠNÚíë˕?ï:?ă?¨	ÀßZد?8¸ož<?¨	ÀßZد?ï÷?¾ÃÕ?"Ç"Bxƒv?œ'…k?"Ç"Bxƒu?ìb[S"?­E°®1ç?¿|ïE%cf?­E°®1ç3FGL J1330.1-7002@s#ý@gÏÀ²mÀ!î'À8ñ'lÀ:óyˆ'!?÷vÏtòÆ1@ã[vsN×@:~äa"ï¿ÝFž<
å¿å$oÅy‹ ¿æÎb("Ú¿å íÅYª°AGNbcuPKS 1326-697?ïìÁ,îj,?duÁ­þLo?c>Ó•Ôã?duÁ­þLr?ïR-iЕ?¦—(Ãêu'?•¼šRÅíY?¦—(Ãêu'?îñ£1=>?žUƒ±Y?¯@åÌì,<?žUƒ±Y?ïýê̜<-?0c%]ü™?0©›"n?0c%]ü™3FGL J1330.5+3023@L­ŸàÛx@T5iÿãzŽÀ:7²€fÃÀ;Þ¬k-v¿Ü E`Ãuq@
P¨ø².@ÌÀÀz&¿é©Æ}Rf)¿åãÀ.XÙ¿â)î`›KK¿ïÿê›ê¬²OTHERcss3C 286?ïø¸ˆÈu?^+þÿû¯?MßìÞ-Ë?^+þÿû¯?îªM*Œ9…?¯Þ
ã9Œ§?¥[-W<g¬?¯Þ
ã9Œ§?íÎB{ÁÞ?¥CÊg}ñ.?±ì!ô?¥CÊg}ñ-?îsÄf´?¢[³ŠÖe"?¨Ã¹Ÿ4·-?¢[³ŠÖe"3FGL J1330.6+7002@]"'þKÊÚ@G\ @hÀ:Ì°G[À;êpçɨ¿ø‡ÁªÚµ@íJsk²?ý~©E¿êö5ó›²g¿Ý3"N*ý§¿Õ	'oß¿Öˤ®YMAGNbllNVSS J133025+700141?ïü1·rø?G+`!šb?>rDh?Ʋ?G+`!šb?ï¾ÁîÛÄ?€†ç&­?€O"|I¬?€†ç&®?閭ȕUy?…Äì'Ó?†^MÚª¢?…Äì'Ü?ïÿXêàMî?3Lœëa?â£öB‰?3Lœë²3FGL J1330.9+5201@[>Ùb…U@Pî`/ë€À:{ÛÑLŽNÀ;ôy±œÅž?×í3¸Fán@öÅ&@ýp N¿êœ.Á¬¿ã†6TÈ%À¿ë{䖱Í?Úö'bñ;íAGNbcu87GB 132842.6+521750?ï›9-&ÿ"?"µ"d=ñ©?‰1´¶@ñ?"µ"d=ñ©?鸞siu?"–¼éæuñ?†û—ã%¢¶?"–¼éæuñ?íÐuk?¦x>Ü/hµ?±¿¤W ?¦x>Ü/h¶?ï§h
I²Z?ˆ½²CmÕ3?†%ü­"i?ˆ½²CmÕ23FGL J1331.1-1328@sØMŸS @H!ˆô'À9ÂMFðPÀ;GÔX²H½?ì,û¶š0@›3\"ë'@ý‰€qÕZ¿Ñ«óI¿áÙRûGá¿ç%RuÿDz¿îÒÁǜG…AGNbcuPMN J1331-1326?ê%êqŠ'?ÃøH鼫M?ÇhV9×Åø?ÃøH鼫M?í§"Ïjv?¸¾^e®Ž?²ÃY"¯ìN?¸¾^e®Ž?çŸR'BË?±öé)ò?ÐÁáZÝzl?±öé)ò ?èŸê'éžT?µÑ¸Höë?̀UôY†°?µÑ¸Höë3FGL J1331.5+1711@uÀLSâÖ@S΀+3ŠÀ9œÔY‰RÀ;ÁÂv1µ…?ç¯hZSÖ@ڍ°e@žÿµ¿è`ñEcG´¿ê<¢óŠ|¿ØY‡±J÷¿ë¶?0†IuAGNbllTXS 1329+174?ï䆡Ìz€?rÇ÷ d¯?ky^3…'?rÇ÷ d¯?íœÅžÍáÇ?»qEŠ•"¶?³Ó	ñÈ?»qEŠ•"¶?îÑۂ`5? ê…˜v?¯âGÙü'? ê…˜t?æ&›rŸÊ0?À¬–c½ßÎ?Ó²ÉÀkŸ?À¬–c½ßÎ3FGL J1331.8+4718@ZDàÚ Ë@QŒÕ£5À9ê¶NÜ&À;úp¨È&?ã¸OO§×@>Âqªa@:ßßùû.¿â"Cׁm¿él®Ž6‰¿çu*ºúÎy¿èëáÁaÅÔAGNfsrqB3 1330+476?ïôZˆtùó?j³zÈʝ†?WJïŠ?j³zÈʝ‹?îë+Ì:Ä?ª–;µ«˜?¡MC<W¯?ª–;µ«—?ï@ñ<á"6?¼›žž±?—áØcÏyQ?¼›žž®?ëM'u"®?³˜Ææo	ÿ?ÃòÉö)±G?³˜Ææo	þ3FGL J1332.0-0508@tـo&)@L!µ'm,À7rá`؇ìÀ:ìZ
7'g@b¶<g[@%8ZåS×@fà‹q¿â†ž²)ªÁ¿ç'EÍó¿ëyÎÎÙ~¿æÚÙë'AGNfsrqPKS 1329-049?ïóþNd$¶?bs3ƒ™ð?Xc7¶"Š?bs3ƒ™õ?ïÉ¡"Ïs?Šù:?'r~?{/=ñ˜F?Šù:?'r{?íé2&çþ?¢@]É6¥,?°·FnÈÀ?¢@]É6¥,?ïýDÙÄՓ?>ˆ¨qÅÕ|?5Ù1ÙSfD?>ˆ¨qÅ՜3FGL J1332.6-1256@sãÛ6†¥@HZ3à\÷À8bÒ°+¬À;eä`gI?ä¼èù©#Ð@Å;'þÿ@V&o¼{¿àí)†°¿çøÛPž(¿äÑ~XºE¿ãR—K$…_AGNfsrqPMN J1332-1256?ïõbs	Ad?bUÁ&VÃ?U;í}5€?bUÁ&V¿?ï»ɳd?ŠÀeØ_q?<M"§?ŠÀeØ_q?îv•[œH©?¡R–ô5e*?¨–ªF;uZ?¡R–ô5e*?ïúmßÂ\?A¶¯VT¾?FH€ö¾ž?A¶¯VT­3FGL J1332.8+2723@Bzòà\̊@T3
ç»À9ÛO
)N®À;꽉b걿ôËvh'¸@;ˆrTÜ%@	4 ›–t¿âÓšj\¿á%$!rk'¿åªøm©?™¿ì­Hœ•¼.AGNfsrqMG2 J133305+2725?ïρßpí?6îdV¶‰?x?vG‰§?6îdV¶‹?ïÒâõô¹?…õ¸í!C~?vŽ…£|?…õ¸í!C~?î–ü?6?¡à™Ã8K?¯<Ä?¡à™Ã8K?ïÿO{¡þ?ꏐK)Æ?‹À=b?ꏐK)3FGL J1333.7+5057@ZÉâ!ȧ¤@P7?úÁÓÀ9PaAcwŸÀ;Çñf	IUÀ"€`¯î@wڿԖÆ@øA?ep¿ãóõ@Œ¿èb+êG9®¿áïZ|ÖÉ¿è(qcDžAGNfsrqCLASS J1333+5057?ïÿè~ÿ~>çéÉöÙ*>çÝ>çéÉöÔÛ?ïØåû7WÅ?'}ނï{?sdT?'}ނïz?ïßnI´O?ut¶ðû
?pHý[%Ø«?ut¶ðû
?ïÿþ|¦
>³‹ïÃ^•>¨5Ÿ_ÇD>³‹ïÃZM3FGL J1335.4-2949@s£àGÓÔ@@
%`ÙRÀ:mOŽ´À;¼Þ&'d¿ßÒkLª'±@iŠ}qð³@_Õ¬˜¥?ݟVg?Õ-¿èjmÜýF'¿ÅxÀtézÇ¿åm›?rAøAGNbll1ES 1332-295?ïÿm¼2¹A?SËNQÔ?Hy¨Ø R?SËNQ'?ïÑ,õ^n3?ToŸ;:'?wi…PÈçh?ToŸ;:'?ïÊ
µFþÓ?v‹çÈZý'?zú¥\€–t?v‹çÈZý2?ïø3$:4¿?K·ïëÍL°?O3o-â?K·ïëÍL¨3FGL J1337.6-1257@t_¿ƒ8.@H/öÿ¦=íÀ8Ȃ•ùÀ;G2¼î¥?÷,\Tiº@l"o^Æ@À
2ˆéH¿åCvè@v¿åÍÎ{½Ty¿é>S-¿ãù;tíŠ)AGNfsrqPKS 1335-127?ïõLŸxª©?ZPI'2\?UfÁª¬$?ZPI'2a?íìq3N˜$?¸°ÍÌ?Ê?°œve‹>Ý?¸°ÍÌ?Ê?îō'ÑÅs?›Dngcø?£§&Ò㨱?›Dngcù?ãŒÔâõÇ?¾ä0ªÀêF?ØæWÒ:u?¾ä0ªÀêF3FGL J1338.6-2403@sÉ}sÉ@BÈ?`h¤À9£ó=yÞÀ;¦Ñb§•?҂Ez2¡@¾]c2Y@œGÿsF¿çoP@ñx¿å6ÎDŠã7¿ê,øËG*¿çïs
q`HAGNbcuPKS 1336-237?︀¿€˜¢?‡sd>9Ú?ßÐÙ×ï?‡sd>9Ú?í*|m¦y?¼%êØvkz?¶¯Œ'ÌA?¼%êØvkz?îÅÍ(ÃC?˜ÓŠž"je?££-sÏËÏ?˜ÓŠž"je?éPŸõõÄ?µá4–ør?ʽƒè((ï?µá4–øq3FGL J1338.9+6532@\Êοìº@InßÜt
À:"H¶R7À<$LaØb,?Ðуüàw@K–ä³s_@(·_þs¿é~+Ž›†%¿ê…ˆ·bò¿ê¼`ºAÛ¿ïû˜Ì·ušAGNfsrq87GB 133543.8+654752?IèQ7?šÄN^\?‡m…ë²A?šÄN^\?ëøso 	Ö?ÁÈXtg}D?À2CØ«?ÁÈXtg}D?îIÌÓ¦Õª?¢@ÈýÍÃm?«c2Œ¥v?¢@ÈýÍÃn?éx±ï²?¹¹\¢ñc?ËÒ8A7É?¹¹\¢ñc3FGL J1339.0+1153@uWŠ?‰'Ë@QÇ€Æ^À9ž}þ2 fÀ;™5<ø®Ó¿Ø{x´û'‡@ªtb¨kÄ?ÿrKl÷¿ÑÙ¸K>~¿ç•èµó¿Ùͳ¥g
Ú¿»û¼WgdAGNbllSDSS J133859.05+115316.7?ïúvаé?Eå¶H?pß?F$¿¹<]|?Eå¶H?pÓ?ï΅Äׂ™?"ž;:J'??x½">³?"ž;:J'A?ïiÌ=
'g?Œñ˜]–èõ?'Æx^[?Œñ˜]–èó?ïìŸU›A?`áK/¤Ùe?c`ªñd¾…?`áK/¤Ùe3FGL J1339.8-0133@to׿¤Æ@M"dŸ¼ÉJÀ:$5a
ÜÓÀ;Ƽ楻ç?JQÝÃ@÷«yjúö@À	Às"7¿Þ£j?^ÿ¿æ(wS¯¼¿ê¥Xl~¿ïÿÒ~ù–kAGNfsrqPKS 1337-013?ï÷ ,v4F?XÚNnÄ?Q¿§—v?XÚNnÄ?ìÁ'®Qi?¼ó/¼ñ¢?¹óêw©?¼ó/¼ñ¢?íQi;Êåõ?¦§Àî]é?µt¶!¨ÐT?¦§Àî]é?ãG†"å‰?½/ë¡/þg?Ùpóº5ôî?½/ë¡/þg3FGL J1340.6+4412@XÀ`#@Qz¾zÀ:'k¢ŠÀ;â;Ñgf?æ«S	@
˨/3Ÿ??þòŽ?žPŽ¿èVŽjø'™¿èè¼J&G¿ß-Ñîäh?®lª‰gAGNbllRX J1340.4+4410?ïùÝÝ?O2ö°<åi?HˆEmȊ?O2ö°<åf?ï Ç=5?–`ð']""?‡Î<pºrà?–`ð']"$?ïYJü³?ŒsÿËÉe?"ܽö i?ŒsÿËÉb?îÝqÿƒß? m>ÖÝjþ?¢(àÎ	? m>ÖÝjþ3FGL J1340.6-0408@tYæ?šIÃ@LF}À?`À:¨nH²÷À;®Ù1_?Õ«j¿¸¬@Œˆ;Î7[?ÿ³»@³Nw?Û#8¥fŠ¿ÒXlŽÚ´þ¿ãÔӍêí¿âˆe邩ØAGNbcuNVSS J134042-041006?ïÔ-ÔÁ\?
줮=¦?uéŸvÑú?
줮=¤?ïCòóÝ?œAŸø¥n2?—ž¡¡"R?œAŸø¥n2?îÈ9B¥ä?›Ï×ï#š?£|kÞ¥¡¯?›Ï×ï#˜?îB Ôi\Ö?›q/·²j?«Õò¹j2œ?›q/·²j3FGL J1341.0+3955@UÑ¿íÁ9@Re¢åx•À:o±,]VÀ<ØúØy?×'þøn@Ÿß…65F@Th€Z¿èôԏ}¥·¿èÓ¾šžÁ¿ÕQ8i'û¿å|i‰'ÿAGNbllSDSS J134105.10+395945.4?ïýҐ¥¹?Bsñû?1kzÒ7Aö?Bsñ?ïxæۛöQ?ŸiY+ÑF?ã$Œ5ë?ŸiY+ÑE?ïy µ®‰?ŠU4φŒ?Ëé\ª.ä?ŠU4φ†?îÅEjo|?˜eH,üÎ?£«©Y?ù?˜eH,üÎ3FGL J1341.5+5517@[ú?̞ª@N3·ßÕ¾
À:aLç9`À<úˆ²Â¿Ç½²"¼¶@
s		i
[@ ^š?¿ä1æ×åÛ¿ì¥/`¯‡¿Óƒ¦K6gÏ¿â«}Ww=ØAGNbllSBS 1339+554?ïþŠ¿ù}¤?2çÀÞ£âJ?'Th%ªÐ?2çÀÞ£â{?ï{ç½F•?šN Æ!Øl?ƒW-^'?šN Æ!Øl?ïqG®å:æ?w€Sß|?'×
#X£5?w€Sßy?著1È`I?°ÁþH?…˜3çí™?°ÁþK3FGL J1341.9-2053@sèàm"@D8ڿԖÆÀ9˜c8´|À;13~²Ž?ëÊ]ð‡MM@-ÍX7úm@/òä¼®¿ã6¢Âž[Ü¿èý,Ñø¹B¿ê˜5ôâJ¿ïÿxÓ·‰AGNfsrqPKS B1339-206?ïüå"1??'å9®F??ˆ×ËfzK??'å9­ù?ï­OÞ-yå?›ŠPå"·?"¬t¡†Ê?›ŠPå"µ?ïjðø…#'?‰ZÞ
3¹?'¡àï[‹?‰ZÞ
3¼?ﳯý®(?wÀN°«†~?ƒ"z6?wÀN°«†3FGL J1342.7+0945@uCoÀL‹Ê@Q5ÅÑqwÀ:a±…H©½À;¿¤àõx¾?ã¤.)wâT@	L˜ Ë<)?ýë8$®¿ïý:]L•?ïàü¬äO¿ã=ô¤"Y¿Ü±z>"AGNbcuNVSS J134240+094752?ïôK«/¯w?X8žÓÇrC?Wh© ¡º?X8žÓÇr??ç² Jmk?ÒM°Ï«\ï?Л¿k%)â?ÒM°Ï«\ð?ï2÷éӇÚ?þ~à¤q?™¡ŏŸ?þ~à¤o?Ô:QWƒy?ÄԓjtþÌ?åâ×T>sD?ÄԓjtþÌ3FGL J1343.6+5753@[xš^»w:@Lñ€@,?úÀ:ÄNÁ.3À<rãLk¿Â»ëˆÏœá@
ÁRæVáŽ@C1¿j¹‡¿ë&n"å¿ëRf¦¿­L‰×•ä¿¿à¢ø*H¨æAGNfsrq1RXS J134357.9+575426?ïøXµ÷€#?o3¢¶U}Ó?N(!ÿt?o3¢¶U}Í?ï"ϕ¿D?"´/ª?"º?Šü/3?"´/ª?"º?î‡e´ë?¯w8þ‹¤ò?¯÷	¤±<?¯w8þ‹¤ñ?ïßx2Ãø?m¬ê¡›"?pCòfžª?m¬ê¡›$3FGL J1344.2-1724@t?Ÿ‡ð$@EՉ?¯BxÀ8ICÝOÒÀ;+ÔÏЍL?÷åKà¤@nŠ§ŽNã?ÿqZÜg¿ÛV×R6Ú¿âÅ¢¦Þ{¡¿âЬkêp¿æ΂&é²AGNfsrqPMN J1344-1723?ïû(Âá"à?AÛLtþ½?C\ôy°ƒÉ?AÛLtþ¹?ï£ 5Iõ?'‹`@ØP?‡7ò¹m'¤?'‹`@ØR?îÈqÛs܄?˜Î"—Z¶?£xâHÂ7¹?˜Î"—Z¹?ïyÎêÞy?…ÕƒI´b?Þæ"¤0ü?…ÕƒI´a3FGL J1344.5-3655@s©[ߏG0@8½¿jäzÀ:'‰)ßÍ[À;¡µç­ù£¿îjÐ;þD$@
ès(ö@t{ \ÁÍ¿Ûêj3œÜç¿â,¦|+½¿ê\Yf,? ÄNE³aAGNbcuPKS 1341-366?ïÁ'Æðú?">|•sq?l‡'·Ý?">|•sq	?ï۟+úe?y÷ÌC+?r0ju'Íœ?y÷ÌC+?ìüöK°Èx?¬t$Œ\¿?¸M¢y¼:?¬t$Œ\¿?ïüi™üžz?:·3Øgã?<³03R?:·3ØgÌ3FGL J1345.1-6224@sQş±á¿ÇõS`œšLÀ7À'°H1ÈÀ:1È\$Ä?óH•$êÆ@Ctà&Ç@É'?_‡¿ÙY4å
å¿çJ'QžX¿è'}Ô¿îßé	Cu¡OTHERspp?ƒ%(1ÐL2?á…m
lí?ï³k_8¾Ï?á…m
lí?ƒ¯ë6ö?'^Ñ6ó³ë?ï±@S%¼'?'^Ñ6ó³ë?µ·òBo?¯°îË{² ?íI­÷²?¯°îË{²Ÿ?¿"Ž}#ƒ?ªDTØü/?ì®=P[?ªDTØü.3FGL J1345.6+4453@WÆ"?@QL`×óÀ7\ahФÀ;|7‰?ô¼
?Ê5@ b¼bÇ@×kŠ½‰¿àš§*s=‡¿åŠÛyŸŠ¿ä¹v?¹¿çwi^WAGNfsrqB3 1343+451?ïýÁAsª›?3fï:P­?1õôb«?3fï:P—?ïÝKçÍ4 ?qΫ¤¦Î?qZe¯¯?qΫ¤¦Î?ïktáEÑ?I…äÊ?''c×Eß{?I…äÉ?ïÿùg¶^>Ô¯¢ô8˜o>Êa'††7–>Ô¯¢ô8œ%3FGL J1345.8+0704@u# ¤<@P‰Î€+3ŠÀ9gíO#À;™x'â3?ê·«ZŒ='@øh‹Ô¡@z¥_ö_ÿڑ]ÈÞ¿ã³MŸ<"&¿ç­Dõä"`¿é†e¨Y®AGNfsrqTXS 1343+073?ïáË&f9µ?pª­‡Tú˜?n4ٙÆK™?pª­‡Tú™?ïÀ4òw?Š 'q†…ü?å†Äþ
?Š 'q†…ü?ì|pY´&œ?©.'^'	?¼}2^Ë#?©.'^'	?ïœæzÎÁA?:ì£'%?ˆÆaLO°?:ì£'&3FGL J1345.9-3357@sºÎ wm@;ÊÀƒoÀ9Ý7iù˜ÞÀ;°¨YOý¿å$Ú#'Cy@.¯KÝy@ºs 
Ìã¿çvE`Ô£}¿è…ù‡¿ÞLs'·K~¿æ
z'R*AGNbcuNVSS J134543-335643?ïÿrÁ¸
ó?5J¢ÐÅÌ?§Èþ¡Ÿ?5J¢ÐÅc?ïÛ$Gñ??z|˲tÒ×?rmÿÜ`â?z|˲tÒ×?ïÜcuîÔ?sÚÝ+*V?qÎE•÷f?sÚÝ+*I?ïó`…¿)?S"ÙðT?Y>ôÛ­×?S"ÙðT3FGL J1346.6-6027@sZýq??ûSA§vÀ8j^IarâÀ:ˆuk¼ç|¿ÖÈ,
=ïé@ƒë²k"@‹C…¶ä¿éªÊ®Ô-¿â7Bvòû‹¿âÐ=õÙá]¿å<'íØáAGNrdgCen B?ìŸOª^É]?¹ON'ký§?»'­	µ?¹ON'ký§?êÔQh<ìw?ͺÄޒZ?Ä®º_N"?ͺÄޒZ?éQPÀT‰?²ŠÈ«jdÓ?˦º¼þ­Þ?²ŠÈ«jdÓ?îýy¹ðÝ
?Ÿâ§lbß­? (d`ò/c?Ÿâ§lbß«3FGL J1346.9-2958@sÐe`A‰7@?_ð€0<À9»éœç+ôÀ;_šÛ¸øÚ¿é'©jz¥Á@œ¨žoAV?û熿wNÁ?çKÑ Ø8¿áµ¤g¡¿ÏUsã/Bk¿Ö¨xÊ/þAGNbcuNVSS J134706-295840?ïøƒê¬?Pa:œ|Ç?OðVQ(?Pa:œ|Ë?ïÙ0ªm
Q?{ˆÝ03$»?sgªÉz×á?{ˆÝ03$¿?ïnyVÎ)?‰'¶gŸ…?'0Õ<¦;?‰'¶gŸ…?ïúÑ¬Ú —?Fû»:Lj?D¹L—}§m?Fû»:Lj3FGL J1347.6-3754@s°>€8Ÿ"@7¥`/ÁÀ9‡"ßöÀ;l³X‡€'¿ññ­w6@rš²t@ñˆŸ¡EŠ¿ä«‹3؛¿çt½ÛB[¿âû¾ŒdŸ3¿í]0©"âíAGNfsrqPMN J1347-3750?ïýÝØk?1ØÜÐü"†?1<§Wò?1ØÜÐü"‹?ïß!Qƒÿ·?{£-çd¬ô?poW>%x?{£-çd¬ï?ïC²æHÚ=?'$Ñc™õ^?—‰£6ä¸\?'$Ñc™õ^?ïÿ³Ì»%?
Õµ‹À?:LÑ6ß-?
ÕµŒÜ3FGL J1349.6-1133@tNßÒc@HhŒŸ¶MÀ8¶ÐE®À;mÖ£æ#¶?éJ½ŸCÛ@Ûç3€`
@"³Gùi¿ãÒ©p&X¯¿äQª¶2½©¿æúC‰Rà´¿êh)pMJAGNfsrqPKS 1346-112?ïá[©oÃ0?j@›•‰å?n¤V<Ð?j@›•‰Ý?ï½RFqƒd?½aƋ¢[?€«ncŸ'?½aƋ¢[?í½Þ2.øl?¤hûq+Ñ?²nˆ<¥?¤hûq+Ñ?ïÿû[[Ì? ©3ç?Š?@""†Ql? ©3ç?=3FGL J1350.8+3035@I²Žÿâ£Ï@S#ÏÃøÀ9
˜®¸À;Â^VY?ì÷"úXÔ¶@«[ƒc@ø¿ƒŽ¿ÛPÎWD1¿çŽ8éð7û¿ã5MTÐ'¿êðw2!ÌAGNfsrqB2 1348+30B?ïý§€ÑâM?8Q²éêšx?2Ãùpí¦E?8Q²éꚏ?ïØ›©NÓ?Øä L³÷?sÿ2+X–¢?Øä L³÷?îLº¯¹¬È?5Èÿl'(?«4Ue3n?5Èÿl'%?ïìÏ1xG6?Z´ôŸjìã?c0·¸ÉŸ?Z´ôŸjìæ3FGL J1351.1+0030@tÛz WŽ\@M⟾vÉÀ9ãÔ;kçÀ;»€õ]县ÁRڅ
@'Â("¯@€Z€ª	~¿åò@òŽ}\¿Ýúê
ò©¿å6èR¿îVÁ(ŒëAGNfsrqPKS 1348+007?ïwæ:Ká?';Ú~+?'8¶ƒßi?';Ú~+?ïÇ9Pù"0?‡vol3u?|cWƒ5èc?‡vol3s?êð•µ`S?°œ(zŸ'$?Ä=©+š~µ?°œ(zŸ'$?ïûx¡mû¾?@Nî¡Ñc?BzH®?@Nî¡Ñc3FGL J1351.4+1115@u·
?‰'Ë@Q2€	¥›À9rÄÞÁÂÀ;G²'a½?ã£àU§@š0øñBù?û^ƒþý¡?ïõ9µÙ@N¿Ð÷ñ‹"¿ÛuhŒÜF迪ªºaAGNbllRX J1351.3+1115?ï¡ÿbü*y?Ž´eõ´[ô?‡€'@õaÕ?Ž´eõ´[ö?ï±ÝúÃ]?"Vƨ?ƒˆ¸O(¹?"Vƨ?î¾&[	°è?–Mþ¼Ú""?¤šOdñd?–Mþ¼Ú""?îëÆ.ž?ÈR$'iø?£×C
?ÈR$'iø3FGL J1351.7-2913@sæ³ S\ž@?ӆ?IÁëÀ9}ÁÕ"äÀ;Œù)L)¤?ÙÃp*"2@ôªaâs@+"¿lçà¿ã¡[òï÷¿åã'*È¿ãÆ_׈¿ìHõV±AGNbcuPKS 1348-289?ïò$ÞÒ]¾?Z¶8MB³E?[¶B[D?Z¶8MB³<?"WL?×Üæ?‹úÔwj,ï?×Üå?ïX÷¦–ù?{3,Ôq?"á=m Þ?{3,Ôk?îúúát\€?Ž)ŒGÅÆ? PQèº7ô?Ž)ŒGÅÆ3FGL J1353.1-4414@s§?Õ%@1>c_Jé2À9YÕ£5#ÎÀ;‡ýgŸKŠ?ÝÅÔGaà½@×Nìő@¿P +"¿é‰–Ü"°¿æåÜ+8‰¿ÝìäÅ<	Æ¿é3ѳ]ÝMAGNbllPKS 1349-439?ïq5Æ÷؎?•Üò7&?'ÙG!îI?•Üò7%?ëÏV\h‹?¾0o;[¨þ?À¦Ž]Ә?¾0o;[¨ý?ìÅ«XÖhÞ?§0ûo
è&?¹Ò¥9L¹?§0ûo
è%?å½»-Þø?¶Î:¤5Ã?Ԅ‰¤Bý?¶Î:¤5Ã3FGL J1353.2+1435@v0":¸c@Qº¿ÖDEÀ9ö†º À;Á¹ã»ü›¿îy­:@Öç,õW@½œÛ½€¿ã.êiž\Õ¿è%ž8uùh¿âr2¹«¿ÞЮ›UÓ¾AGNbllOP 186?ïÿÓçHÙ³>ôøA*ŒuZ>ö["&Ø>ôøA*Œu"?ïÐàF‡?…ó))
ý?wðý\»ó?…ó))?ï¿M]éÒ?'>…hgÅ?€,¨¸…‹Z?'>…hgÀ?ïû—ŽÙ±,?@ oåÌ?A¡Ä™;S¥?@ oå®3FGL J1353.5-6640@sP @|ÇÒÀ#7À5º¢À9]ÇËÜÀ;BЉï•?¿˜à«ù@œuÁù	?þ{``½Úì?¶Ú¡Ì˜õZ¿Ó•nË©zý¿à÷†<x4¿Ý'û»¼rüAGNbll1RXS J135341.1-664002?ï¥tš0Où?‡Ž¹v¤1Ô?†¢ÙsìÒ?‡Ž¹v¤1Õ?î_³snSJ?·ÙŒŸYߗ?ªÈÉËZ?·ÙŒŸYߖ?ï­úõT?'˜—Jö?Š@¡U~?'˜—Jó?ïk¡Ã
ž?9Ëþô ?'‹ÇžL<q?9Ëþô 3FGL J1354.5+3705@RišÀ
F«@RXŸá²7À:|¼A%À;üÔyixj¿±"Jn@
(oxùt@LŸ•Ü÷¿Ü$ÖN*ÛK¿áµ¸r©¿è†ñêR¿ßó(ôy-AGNbllFIRST J135426.6+370654?êÐÜÝÜ?ȇDññÀ?Ä¿ˆŒˆœ?ȇDññÀ?áþ ?¶yÆf&"?¦"wà?¶yÆf&"?êW¬/àpý?»ž!
/G ?Æ¡O@~<?»ž!
/G ?ìîÝ+Ö£¿?®ógÇÞL?¸‰¡Jâ?®ógÇÞL3FGL J1355.0-1044@ts<`Ÿ@HŽ¥?À	pÀ9@'
´©À;†ºö
³¸?ì³Jð"'@'È"ÙÁ@ûÿë2>¿à\ùՐã	¿åÞcK†¿éGl°ØO¿áñ±Òº;iAGNfsrqPKS 1352-104?ïý
ÐÝ?8ª'ü&?7©ñM€?8ª'ü&'?ïºG•ôj?ˆ¿ØTk•?n'å|†?ˆ¿ØTk"?îºV²yÎm?˜Úœ&	šj?¤Z"Øc??˜Úœ&	šf?ïߦóà#?gqŒ³a÷?p,†òï?gqŒ³aò3FGL J1356.3-4029@sÀüßï¿@@4¹&Ÿ¦ùÔÀ:+qøjàIÀ;®2Ì&°¿áÆ(Ûìz@Y0‹yp@{P@4M¿èî)jª¿â°´ a'¿çÿ'z9ÏQ?Ô6aË÷åªAGNbcuSUMSS J135625-402820?ïáGy¤‡S?qfÂéÓ6!?n¸†[x¬ñ?qfÂéÓ6?ïÞ¥
lþ?z>}Ý"?pô­zɁ?z>}݈?îù1ïHÙ²?—»½²í›? lárdë?—»½²í?ïûõ)?Aâ—ûâ8ª?B+‹£_J?Aâ—ûâ8¦3FGL J1356.6-6428@s^-••Àð[ b 1À7ær/ÈEÀ:µ'v©V?ñ+$®¶j@U$Zþ@|'@Y·V¿äOEAÊòú¿é>'úeƒµ¿èyæ¼É/Å¿ëÇѺ66PSRPSRPSR J1357-6429?ÍcáK†f?Æÿ)cÔ?觭f~?Æÿ)cÔ?§À—'úm?½ÿ¾l	Ñ?îƒö†ÐY0?½ÿ¾l	Ñ?ØU9>Ï<_?»Ujxäij?ãÕc`˜aÑ?»Ujxäij?½,NŽ?£N
*k?ì]z}Ýö.?£N
*k3FGL J1357.5+0125@u?€ß×@MæÃ`<€ºÀ:p
TÙÀ;£'wŒ(˜¿ÿ;WýB
'@x_ã@#lYA:¿ézcp½­J¿ß¿üõ‰"y¿çˆ\›Cé¿Ä…âØ|ÙDAGNbllRX J1357.6+0128?ïЪ‡€§r?~7wŒ,?wª¼?¬GO?~7wŒ.?ïËVÉ:ƒÃ?‰í"êž>?zT›b¾ê?‰í"êž=?îñ¢Û¬Lò?˜¨·ƒæ&? åÒE;0Ö?˜¨·ƒæ&?ïÿ¬4)Šr?¬Ðv‹?òõc^Ç?¬ÐvJ3FGL J1357.6+7643@]ƒ5Á'ì¯@CâÍÀÓgÀ9Gêz\½À<'ÇÅý?òjêD+þá@ŒgH8¨é@ßs¿jc¡¿åq8b®1¿äÍ$oËë¿á Š.öN¿ï ¯?‰AGNfsrqS5 1357+76?ïÜ1ê3Ú?tM½ÄŸ	p?qç
øfd?tM½ÄŸ	p?ìõæ?#è/?¹êãé½K?¸PÎ྅?¹êãé½K?ëX›ôæ´?¬|R¸:{X?"ä,e.?¬|R¸:{Z?éÙÓ¤ÈQÖ?´Iv—<l;?Ș±lÞ¸§?´Iv—<l;3FGL J1359.0+5544@Z  ô×®@Mr /µÐÀ9Nû'²õ‹À;ô4-n¿ð-âPíƒQ@Ïl®)±@½¢À^ÕM¿æI6¦kuU¿ä
"£`¿ëJ.‹>ô¿æ…=å):AGNfsrq87GB 135720.6+555936?ïù‡ù
mT?VÔìu›"à?IàÖJ° ?VÔìu›"ß?ïË3gGÐ?‡¨Eø9{=?zfL\ýÕ?‡¨Eø9{??ï?µÖc&?'Эêý½?˜	E3Ÿ›L?'Эêý½?ïþyª~?1ÓªJ˜Ä?.heX±?1ÓªJ˜ÄD3FGL J1359.2+0204@u+é>ê!@N矶êÀ:Û/fÀ;"ãiÇC÷¿Áò–‰KT@
éá·?œÎ@©Ýÿ¥G¿q&ʚ˜Î¿äk8>¤šB¿âÊ˲4^ñ¿ïê…¼AGNfsrqPKS 1356+022?£'&A?¬_ÈÍàÛÂ?§¤¥Æݛó?¬_ÈÍàÛÁ?îO´!×½j?­j<¸‹­ä?«½â")q?­j<¸‹­ä?éfH6Ï*?´™È4Ù}?Êfß$çX?´™È4Ù~?íÈ~c†ý?§‡ý"W[â?±¼ãÈŽ?§‡ý"W[ã3FGL J1359.9-3746@sÙtàM/@7#Z0FðÀ9iÀJÞJ¤À;s&îR{?è–îÞ3kV@Z?A3@0rÀ;ïÅ¿å7šÆ•P4¿æ˜û;A–ñ¿Ôì·p;Ÿ¿ÞPF¼v/AGNbllPMN J1359-3746?ïá:x¿AÁ?n[–ßÈ?nŇ@¾@?n[–ßÌ?î۞<Vv?©5I6°-?¢F7ꘟ?©5I6°-?î¸\yªÄÔ?˜¢º—é:?¤z8eS²Ó?˜¢º—é:?êX{ëw×Ì?³~¯ 7"?ƞR  Ô?³~¯ 7'3FGL J1400.5-1437@tnݿη‰@Fßä׆À9e=?&À;Š²@YŒc?ñáÐd±ÛZ@
ZMÕ ÛØ@d§ê9?«[ž§~¿á3(N±F'¿äÒõÚ~|¿ïÿK3PSRpsrPSR J1400-1438?±G¡TPž?¿	¿î^'?í×Õuì>?¿	¿î^'?­ÞWòlÆ4?»Â®0j\?î"€Ù3œ?»Â®0j\?Éá·úJ]?´(!mIÊ?里^mi?´(!mIÊ?´§/Ì>¬?šÆð+Pã??íkx*?šÆð+Pã?3FGL J1400.7-5605@sˆ€CR@ïI$À9É÷/væÀ;!€´Ê?ç/þÛgÅ6@èhÜ7xè@ù{ßto>¿ä;v€Çˆ¿èl5†Ži¿ä~ÒJ‡…¿íˆgS\…AGNbcuPMN J1400-5605?ïéÂQbr?aßtä'1?f=®ú¶?aßtä'6?ï'®x—?œYìJ¢€?
Ê<í?œYìJ¢?î8Õø]]?˜š‹h§å>?¦,r z*,?˜š‹h§å>?îÖÂtÀ¡?‹ñWÈz¢Ö?¢"سõçõ?‹ñWÈz¢Ö3FGL J1404.8+6554@[àE€<ÑB@HÇÀgnÀ:"¤?
À<3ÿn	È׿bÓ(iª5m@ªÕ"ð¸9@¿	 g¿¿å•›Jý1ø¿ÝWp3®¿àþówJS$¿åS"ÜôWAGNbllNVSS J140450+655428?îãa2O
?·"VÈÒ¦?¦ñÉìÛ0?·"VÈÒ¦?ïïBÉ?£tˆTX–÷?œð·¦ï?£tˆTX–÷?í¨-»/s&?¯?ôhç¤?²¾'&"fÞ?¯?ôhç¤?ï_
}‡õ¼?ŒA=Ž™.f?"°OH—?ŒA=Ž™.f3FGL J1404.8+0401@uuS@N¤©@NØ_¨DÀ9±ŽXó·À;šAÿŽÁ¿þöFÖ~&w@
'ZÀëÃ?ÿ¶MAQY¿åüc«ÿ€\¿à<2m»oW¿×ć^X¥Þ¿å2'#ÒºoAGNbllMS 1402.3+0416?ïâ¯9Ñp?rE²Ïx…?méPÆ.¤?rE²Ïx"?ïËyvò`á?‡ë"Ä› d?zCD†Ï˜?‡ë"Ä› d?ïW†§Ó|`?ûÍ8~ê¤?•+só?ûÍ8~êª?ïýxvÇ!
?FØâ²ñÛ²?4<IÆ÷Ÿ6?FØâ²ñ۝3FGL J1406.0-2508@t9}sÉ@A[Œ@ÃÀ9¹FMÂ*²À;ƒÈ¸kù?…°ýEÂ@"Mië?þI`½¯ù¿ÃMW<¸ÿ!¿â˜šÿR䇿Æ^,h
L׿äB
s¨fAGNbcuNVSS J140609-250808?ïîÍ4¶ú??mp*ØÿïË?a2ËIÀ€?mp*ØÿïÇ?ï'÷.'æ?' (Û½æ?‹'4_Fô?' (Û½æ?ï)ðÎÊ4ê?'jmœ
ó?šÁæ&¹bÂ?'jmœ
ó‹?ïtßÁJ)ñ?‰éÔÂÁ¿?'dÖºÁã?‰éÔÂÁÁ3FGL J1406.6+1644@É?áAy@QoÄ`Á
À:ž°²ºÒÏÀ;ÅbôÁÞ\¿Þe¼S>&½@ÁÁnSñ?ú[~ Ai?îôÕÄ¿â–û†è¿Ý	º&_˜Ê¿¡ï¢î4¯AGNbllRBS 1350?ïþFâÀ?.ι^ÚR¨?+žÑßì´?.ι^ÚR6?ïÐ	' Éà?†UЯ ÈÁ?wû6ï›?†UЯ ÈÃ?ï^U¥›J­?Ýùû A™?"5KL–ªz?Ýùû A?ï÷ÊØN©?KÖTàëA÷?PkàOb®1?KÖTàëB3FGL J1407.7-4256@s×àßÞøH@1¯3+¦À9½ø¨ó©°À;˜êË»TÕ¿óDçÈüˆ§@ÖðäJ7@Éd~Û¿â}^â'kÄ¿æ0²
»¿Å%Þ®CM¿ìR€‰ŽoÖAGNbcuSUMSS J140739-430231?ï|¹ð(<?˜Î<Ä?hÁúø4?˜Î<Ä?ïÉÄÕú+Ü?ƒto&ý?{•êš?ƒto&ý?íP:&t¼?¥‹4d¥?µ~.ÌZt?¥‹4d¥?ï÷b2â¿N?X¦¦Ñd?Q;š:cî?X¦¦Ñd3FGL J1408.8-0751@tÝ ßÞøH@I'æ@;YrÀ8|«ÆÂǐÀ;SÀ'U'z?ïM,6G@u ,°¸@	ä ¦hµ¿âºp‰ ¿ç-þQ:kr¿åÞ°Á¿äTjõ䕎AGNfsrqPKS B1406-076?ïýÿìƒ4ÿ?7ŽÓA?0›æX?7ŽÓA
?ïulÁmñ³?˜<ݼè¹?'RgÒAɊ?˜<ݼè¹?ïrð¬È…\?Š'°ÌýW?'¡êfïT·?Š'°ÌýX?îpútÿŒ®?—m–%ý…?¨ðX°50?—m–%ý…Œ3FGL J1409.7-6132@sÝàP7P¿±9RŸô¢`À7|[TŠœÀ9±]ïŸ_¬?ð™!ï¾ê6@‡Ý­oº@ïÀ—µ>¿âÜÌG€&¿á£Ó<Ÿæ¿å°å"«s¿ë†}]#PSRPSRPSR J1410-6132?WŽ§¯&å?]±ÝH½r?ïô8¬(pm?]±ÝH½r?oöŠ(	{ß?~[6÷:?ïà	u×öƒ?~[6÷:?·í—I–?§"ô8=?íMVßM?§"ô8=?«÷Œ'?žYÐ\+M¼?î@—8Ü?žYÐ\+M¼3FGL J1410.4+2821@DÅk 	ŠÃ@R4¿û-2À:IÚÓöÀ;滵MTG¿÷ÖÞñ'@
‰%Bû?ÿ˜ nJ¿ì¦½!Å2á?±šnHæ\¿ä'ø<‰•¿ÊŠûô$!AGNbllRX J1410.4+2821?ïÉ ú³Æ?‹‹ÈUº?{/'¦s/?‹‹ÈU»?ïÇä&[R?‡ñ´˜ër?|
ìÒwV'?‡ñ´˜ëp?ï"ç)ô?–p•a<¿R?Ÿû£ßa"?–p•a<¿R?ïûžÙ£û&?HsÈÑM×h?A"™peE?HsÈÑM×h3FGL J1412.0+5249@X‡, zû@N  	ö#À: H{™ÔRÀ;ûã±ëŸ÷?åϐé>?@éþ³ú™@L_ª	©¿ædÈÉ\Ï¿ëKúo¿ä¸%3ÒP«?Ɓ¡?Ö.ËAGNbcuSBS 1410+530?ï÷Øø?aBª—u?QÃÍØN#?aBª—y?ïyjæ§?£ÔÛJE§F?Ò½Î+4?£ÔÛJE§E?î"D¯ì¸?šÁH*È>À?¦»¿å4œ?šÁH*È>»?ïSå7¨ùf?—P%ÉÄöx?•ƒY
àÓ>?—P%ÉÄöy3FGL J1413.2-6518@su`4óþÀ8Ô ~$ÉÀ9 ½zIrÀ:ï-؀_6?äI4Þ%‡@Ai×µ@j±€k^¿Ô®<ƒ¾æÛ¿èå*¡¿,ü¿å«ˆ†½Ò¿ã5ގ¿ùAGNseyCircinus galaxy?ë#Ì^$;7?£K û±?Ãp·o%?£K û±?ëþ•ÆÎÆ?Å°º/ބ?À¡¨äÄä?Å°º/ބ?ç3ü¨«gÎ?½ÑÖ¡=a?ј®©0f?½ÑÖ¡=a?êú_'"É?¬ÿWåÃí?ăc­°Û?¬ÿWåÃí3FGL J1413.4-6205@s…ÿ@O¿çP®-ø6À6WQ'©"À9íi›¥"@+Hˆ"ôF@»¦9:3X?ÿôÀŒÉ¿Îà%¡¥,¿à;5Ý\'¿ãÇÇ)þ3Ö¿ìßØ/wåPSRPSRLAT PSR J1413-6205?2Ъ3°L?0¥³ö	U?ïý¥ê¿Œ?0¥³ö	U?à•#Ť?8ë›Heù?ïÿûWöã?8ë›Heù?t#ùP"o?c)~;3?ï×ϸ
_¼?c)~;/?!W·\¶t?O+BP`Ì?ïþꄊ>Õ?O+BP`Ê3FGL J1415.0-1001@tæÿëJ@G׌àM³À:1¨oö2!À;¢\Gÿs?ñÇQ'ºÚ@I O–@I@ô\ mf¿æV*ۏ¢¿ê&J¿éÔ)¯É(¿á»z	äãÍAGNfsrqPKS B1412-096?ï
¶5Ïr`?£ÖE1âÊ?žI9F³ñ?£ÖE1âÊ?ì¼eü²_¾?Â8ƒ¹‹¾Ž?ºÐm?Â8ƒ¹‹¾Ž?éÉÒ\Ê¥›?°Óá0@Î ?ÈضŒÕi™?°Óá0@Î ?ݦmQ° %?ü­<o'·?á,ÉW'ïî?ü­<o'·3FGL J1415.2+4832@VÖÿÚ@S@Om€6EÀ:9¤$èîÀ<™RKý/?ÒõË'tÚ@çŠizî@Y¿Xš÷¿ìX¬Œîîé¿ã€—.5¿Þø¢æ@ޏ¿é«ÊCZ°AGNbllRX J1415.5+4830?ï•2qZSà?–8Œ>ú¼?Š³c©kŽ?–8Œ>ú»?îõÅß³=o?«ÇêmÇN? £¢Ì)?«ÇêmÇN?îy¸™4¿Þ?ž¨´øꆞ?¨dvl´?ž¨´øꆞ?íZü"ÔW)?¨6UXæsÎ?µ(Y]F´?¨6UXæsÎ3FGL J1416.0+1325@) -@P}MÿÒ³—À9·Ät8·À;ÃûkEÉ8¿ä‹×<oûn@°1вŠ@èS`¥1R¿å4—Ö á¿ã2δX¿ãp	Ö©¬¿çˆ\¢d»¹AGNbcuPKS B1413+135?ïþˆ••åP?2ÿ´=Öœ?'v¦¡«'?2ÿ´=ÖÜ?ï¿(±"Ù?ŠHZ=ó?€5Ó¾Éå?ŠHZ=ó?ï¦æ÷ˆ·"?"´2•‡?†FBÒ7b?"´2•‡?ïô^<¢Hm?Uõ7¯–ãC?WC†»o%Z?Uõ7¯–ãS3FGL J1416.1-2417@th€àe0@AT"¤%À9éé8=^/À;ŠçɨU?ÁJdI£@
ÕQßñ—²?ý¤ã!"ž¿æ´ëQ+Ÿ¿Ôàña׋m¿Ñ¾Ò¬=hʿܱѪAGNbllNVSS J141612-241812?ïõ¥¼(¨—?VnÄy^3K?T´‡®®Ô?VnÄy^3D?ï¶@ûcæ?†‰Ø³«AÀ?'oÁ§Q?†‰Ø³«A½?שׁQ#™-?€åõPë¨&?"Õk·´Í?€åõPë¨%?ï›%^O¿2?}Î_«h?‰6¨l3–?}Î_«h3FGL J1417.8+2540@@Âõ`iÍ#@Q§š_ý–™À:@җçè²À;äOªb>¹¿Â>­"@$f@wBIP«ê@O=f'@¿ä=ÆҌÕ;¿ç#HÖ¢Rj¿ÐèyïÊŒ¿Ør%åumÉAGNbll1E 1415.6+2557?ïþ¤uHŒ?1UO(dÇ?.Õ¸«w5Z?1UO(dË?ïČɭ<(?ˆö/:Èon?}¹›)aì`?ˆö/:Èoo?ﳝ:ð«É?€öüc|?ƒ±CÕ
£?€öüc?ïØn¼¿i~?oÚå%+;b?sÈ¡ KA?oÚå%+;g3FGL J1418.4-0233@uYO d#–@JÓ`IôÀ8C¾vÈ´9À:§dd-§?óșSù|X@¿¿
œ?òº0»3È/¿«1œÜ]þ¿ÓٖG2L6¿É|µ»ÁÀ¿Úñ3ÉÜžAGNbllNVSS J141826-023336?ïòŠÏÒB"?q«ÓB+AK?Zê`[zڄ?q«ÓB+AM?ï'¥=y¢?£]z#Nm?›X^ð˶?£]z#Nm?íQr?¨Å¼L@>6?µpŠûk|m?¨Å¼L@>6?ì]Å%入?±p2óFøê?½ÖÐÓÒÔ?±p2óFøé3FGL J1418.5+3543@O˜XóÖ&@Qe`&±EÀ8Ml+¢E:À;<º¾­OY?ê6©a…"Œ@<cϳ1@w§€)Ú¿á7ñÓdÞ¿áQ<{0wí¿Ý&¤ãu¿åh^©AGNBCUNVSS J141828+354250?ïþ¬˜K…¥?$ˆÌlÇ¥?%6{G¥¼B?$ˆÌlLj?ïՀ4F،?…CÈò¬?u?åܓ¹w?…CÈò¬?ï¯9UÑ=ö?'YQP€ô"?"1ª‹°'y?'YQP€ô…?ïÿåM&å>ó'!ŸgN™>ê²Ù÷à‰>ó'!ŸgMj3FGL J1418.6-6058@s•òä?À« ƒ¥‰À5ä°S'ˆÀ9m˜‰Ï@>Î 3ý@¶ÓŠ"Õ?þäE,ã¿ÉrÔÚs«¿â"èCî
Ý¿æl@·øvÁ¿ì·ã8ÉöPSRPSRLAT PSR J1418-6058?Sûøž;þ'?V<åN
«ò?ïö°â?V<åN
«ñ?,Ž#Až?@°Æhÿ
l?ïþ7ϋï?@°Æhÿ
l?‹éïÀ@…3?û–òúêª?ïX@þýë?û–òúê­?Hi"Ä?JÆÁ(é-?ïùå›ÿÚÏ?JÆÁ(é-3FGL J1418.9+7731@]@ù?ò^W@CK. &{•À9óË!ÑáàÀ;àƏ›éÖ?êªÑI´)@'œH 'Â?þ€*Ÿæºµ¿èr|Ë$#¿ÖH
y©ÿ¿Û¼^ØÏ¿à¼#p·<AGNbcu1RXS J141901.8+773229?ïÔ¼wÆ©?f튎<?u¡Äù«ó?f튎<?ïŠeOR? ç4v>¶?œN¿óV‡? ç4v>¶?ïvÿ€U?–´'íÍ?œñ OõX?–´'íË?ìæv÷Xä®?§97ø`n¤?¸ÌHE8ڈ?§97ø`n¤3FGL J1419.1-5156@sÆ>KZ@!?" ÔÇÀ99rãLkÀ;¦-?Û¸çV96@
úßڛ—@LÀL
ð¿æKQýE2¿éH<Mtc:¿íù•©
³?¹Éi–AGNbcuPMN J1419-5155?íûèêQ!º?±–ðä€Ïø?° ¸­vò6?±–ðä€Ïø?îzÆ%âDÀ?½,IôžŸ[?¨S¡Û³ý?½,IôžŸZ?ëN"Ió?±|Þ·~L?òÅîÙÀ2?±|Þ·~L?ì2RESì?·#Ã^)œð?¾mm×=`§?·#Ã^)œð3FGL J1419.5-0836@u
–Óõ¶@H0%ŸÌ¹'À9ñ|¯~À;~i%]‡›?ópò~$@BwsÔä@)ñŸj¿ÕÐÉöG‰E¿äZÚŒ_¨¿ç4L—wV¿çd^¾/AGNbcuNVSS J141922-083830?ïå<@øÁ?q:ïâ–$¯?jÃþ¿>'?q:ïâ–$²?ïòàž?"O«Ë"H?‹þGþØW?"O«Ë"H?í›"Å-B?¥äŸÛBàú?·s#a֕å?¥äŸÛBàû?îéNÞà«?'t2Zr*!?¡kâõ6?'t2Zr*!3FGL J1419.5+0449@uâê@M®Q¿æ4}À:•ža÷À;¾Љð?Ïêé˜_ˆ@
&Î 4?ümá]?ìÅt¾:Z;¿ÔÂ
@ºt¿ä;ÝâÚç?ÔÁš	.ÏAGNbllSDSS J141927.49+044513.7?ïÈïâ†v›?ƒÐ‰0ÝË?{ˆ¼Ä²‡?ƒÐ‰0ÝË?ï¶'Œ¢?cÀ¾å6,?'~Û\ÿ—5?cÀ¾å6,?îµâ»äñ8?™÷{÷Oš¥?¤¡ÔA°ìh?™÷{÷Oš¤?ïÉnøg£?yk4õ&þ?{HƒÌ.8ù?yk4õ&ú3FGL J1419.8+3819@QlT_Ó¥.@Q³çüÔÀ9˜ov°`…À;ãžs.?ÚÊ4Sf%ñ@
qœ÷GÍ@êÃyíؿݺÈÆáY¿æHÓ¿–i ¿èÀ…tQ¿ãäVpœlªAGNfsrqB3 1417+385?íÙêj´Q?µ¹uqx?±7P¬ª]x?µ¹uqx?ëö©L€?ÇÍW†%Ìe?À'Ï©ZÎ?ÇÍW†%Ìf?ëFXÐZ?µî:ÂW?ÃÆ柴¾™?µî:ÂW?ãöcä˜]?Â9^áӀ?ÙÆ86ÏE?Â9^áӀ3FGL J1419.9+5425@X"'`4P@M"ßµ§íÀ9*X R…ßÀ;Õ»¢ç¿À¹u³q˜/@©¤aÒ#@u¼ '+"¿ä%bf_¿å -êÉâã¿áC×ͪ¿äÉâb=ëQAGNbllOQ 530?ïÿa±–/<?*¬—­X2?ÉÍ:iÆ?*¬—­X4?﵆/ˆyû?‰Þ™™9 ?'žtá€ä?‰Þ™™9 ?ïÐôsõž¾?y«wR¦?w…Æ0¡^?y«wR¦?ïåÿo‡•?dk4¸@«?jxíjï?dk4¸@§3FGL J1420.0-6048@s˜jŽ:Á?Ìb'KÀ6Œd¤ÅFÇÀ9-#'Õ?öèË°íô@& ß²C@õž_§'¿äø²Ñ‡¿á—~ôt(¿åV+8p'¿ê[õ¡âéPSRPSRPSR J1420-6048?r`¼ ¢?t˜ªÎ¡ÃŒ?ïÛ>‡é¿Û?t˜ªÎ¡ÃŒ?‡‹.#ýx?–šT=­?ï¡ÓG›p	?–šT=­?®ûÓ_ý"r?¢Øn*ö?îBÊ-Ù?¢Øn*÷?ºº"P°d?±@ÅÆñ͓?ì½h¯uéô?±@ÅÆñ͓3FGL J1421.0-1122@tõEߨq¤@Fäq_¾¬yÀ:ï!‹kÀ;¨ñ՚Ѩ?â¥hF‡Æ*@*¦ò—@ƒ{À?˝?ïðHöF¡X¿àKz'°§†¿Ü"ŒM¿é—ðJ'"ÞAGNbcuPMN J1420-1118?V
?ƒNãÞüg?~¾±TúŽ?ƒNãÞüi?ïAY»º×?œÖ"«×S¤?—ÔȜ(¤ù?œÖ"«×S£?ìÓÓÒþdÚ?©'·»Ÿˆ?¹aahÙ,?©'·»Ÿˆ ?î¨0è7F"?™[ì©p?¥|ñ|‹–Å?™[ì©o3FGL J1422.4+3227@JÅ`Iô@QeæÀ:s¬ ›%À;ÿÀƒé.,¿Ù8Uj'Ï@­¼Åd#@zIŸÜ(à¿ê,‹5¦ú¿áØ:å6ُ¿äoÙ1^¿ïý¤µÎÐÕAGNfsrqOQ 334?ïºw-x}?‰Á­w™»?b=4¡àµ?‰Á­w™¼?îüŒnt7?¬›kMbôc? >G9¼'?¬›kMbôd?í:O"`dÝ?¨ÊkŽr\?¶-ƒ\üÙ?¨ÊkŽr[?ï¥'ë]?—õE…`?Ÿ["Y?—õE…_3FGL J1422.4-6137@s˜^`=Wy¿ä¶ŸÇ±À7¿—02ͳÀ:c""aSØ@ðfôUÒÅ@BŒ:áRk?ñ¦õºgš?ïùÎدs?¸žàLÓºŸ¿Ûæøݽ¿ëk$GSšPSRPSRLAT PSR J1422-6138?~ÜÊ«(?€±GnÁ˜?ïÂFj©¯ß?€±GnÁ—??{Ò5XPH?]ŸŽšP~?ïü…¹Tõ?]ŸŽšP~?´Yµª#-v?¥¥'õQ?ítÉJ»šR?¥¥'õP?}€wÛº{?u¶©AX?ïÄÿH‹	?u¶©AX3FGL J1422.8-7828@s9(€QÉ÷À0p‡ÀSAÆÀ:VD& }¹À;µü‹×97?ï@"§;@"Õxíҁ@\t_£S­?Í$Ø5¥m&¿ÙÆñ§³Ê¿à\2ce¼¿è)'KãòóAGNfsrqPKS 1418-782?ï§îñ$>?'J·?†C¶ß°€?'J¶?ïQä
'ÄV?¢çÿÃÍÈT?•Ã~MÇuU?¢çÿÃÍÈU?ìï˜ó?ªî7«¦M‹?¸ƒ?Pc‡G?ªî7«¦M‹?íp4¶Z?žõr¢ ?´~_zM/Þ?žõr¢ 3FGL J1422.8+5801@Ys´á¼©@K˜Z?çvœÀ:‡ëÚ¯
ŸÀ<!µ±þm?鵡,éu®@
V;Í5¨X@$û_\[ö¿ì¾§:õ|ø¿ì^êв¤F?â/ãu/×ß¿Õg¥<AGNbll1ES 1421+582?ï÷z'"­ ?`EÅ¢.#?Q
úØ¥À?`EÅ¢."?Iðâ?"b%ÒLq1?ˆZ-ƒÇ~?"b%ÒLq1?îâW'tê£?š¶
úÞt?¡Úˆ±UÃ?š¶
úÞs?ï¨ûBÌً?šù
È®?…Á/Lɝ™?šù
Ȭ3FGL J1424.3+0434@uø›@-¹@M1πsÝÀ:…Óé÷€À;Ê(X
Þ¿Øñû	öùÇ@½Ta$X@㽀~•‡¿Ý÷›ä…È¿çñsÛDî¿åh†0ÂQ¿á¼e¦ÍߜAGNbllTXS 1421+048?ïõ–§…ñP?Yç©xãÍÂ?TÒ°ô`|?Yç©xãÍÆ?IÒ*f?â¢ùíçM?‰Ù-‹uf˜?â¢ùíçL?îjCßÖ~Ï?¢ԱݠU?©[˜?¢ԱݠU?ï¾³å6‰?v×É3õË?€S˜²]m?v×É3õÉ3FGL J1424.6-6807@swp€0<ÀEÔÀH^À8l›
²áÀ;/*Ê®å?ð>¢ýñ]@{L‹Hóå@I½ 1xÉ¿ã1=¦9÷.¿ç-³;£'Œ¿çÈoè<·8¿ê™¼å¬ :AGNbcuPKS 1420-679?ïÛªþBÜs?v&7cýYB?r*€Þ'Æo?v&7cýYA?쀲/[]f?À(¿÷>oü?»ún…%Í?À(¿÷>oý?î}ˆ"'Ó?™&¥e ?¨'}ÖâÎ.?™&¥e"?ì	$0ë	T?¥µÓ-<?¿¶Þx§µ\?¥µÓ-=3FGL J1424.9+3615@O¼ÿëJ@Qâ (zÀ9]Ô´øš±À;¦V6mzWÀ48éU™@UòŠ÷jZ@ÄÓ_ãëL¿×Gž?È¿å›ÖDg/†¿áaÍm-8¿ÕŒ8ôΖAGNbllFBQS J142455.5+361536?ïûûo
‡?BÔ§–  ©?@šCÉæF?BÔ§–  ¼?ïÝm"±z?'ËñT4#•?qrI=§By?'ËñT4#•?ïRú;œ"°?ŽœÑý~~!?• ¸ŒmŠ?ŽœÑý~~?ïÿÿæªæ>‡ UEb>iUÚ¦~>‡ UE+3FGL J1426.2+3402@LÀŸ¡ñW@Q ß@wÏÀ:R¸S™HÀ;áðT'QÌ?ãÅ-žÉ¯6@
SÛ&Éï?þÞ%ÀÕ?Ù¯L+§¤¿ß Ëkg›ß¿ÓeØÍ¿æ2¹˜½|AGNbllRGB J1426+340?ï†íÛ¸Ö?'Tҝ?ŽD‰Êy±?'TÒž?î˜÷(i€÷?¬!'QæäÒ?¦pygð†?¬!'QæäÒ?îÒŽÒ3Ü?›nw"S|·?¦ò×ÜÂJ?›nw"S|´?êúõX|ý?±¦áôƒ«?Ä+îž?±¦áôƒ«3FGL J1427.0+2347@=}z °P@QúÿåþÍÀ6¡H2ž¸½À:ÁÅìß?é×Pô0¶N@d¬Iõl~?ûŸD®'û¿ÖÝÕL'î¿Üãȗ3ó¿Ú#¹m¬<¿Õ¼aÛ(AGNBLLPKS 1424+240?ïJ¹Fócj?¢^ÏÛ¹Ã?–¨×!"'™?¢^ÏÛ¹Ã?ïÐyXAc?…5P"å(?wÃpSßN/?…5P"å'?î@`$~|ö?¤¬'eMêð?«ùý¸0 ?¤¬'eMêð?ïÚ;v:q?sö
/ÒÇþ?râDâ±GÌ?sö
/ÒÇù3FGL J1427.6-3305@tRÕàqÅ?@9—3 ¾¼iÀ8'ÖJúÐÀ;[Êò×ùQ¿ÔÚÍÀV‹—@»66ó²@XØ\œ8¿äB2øOÝc¿æ[k2þÚç¿æÍõbµ#¿á|RAAGNbllPKS B1424-328?ïþÁ+c:?+ÐL¾vþ?#îÝIÌk€?+ÐL¾w?ïÝjÚöâ?|d<OÓâ5?qJ'"øQ?|d<OÓâ3?ï¯Ä¶|úQ?ƒ"؈ö°?"Ò`Ákž?ƒ"؈ö°?ïÿ[¥3?EúΘ™\?ŸYŸ*H?EúΘ™é3FGL J1427.8-3215@tYªK@:W– hUTÀ:apÑ#s£À;±,±8ò¿Ë¯iU•D@¯~瑟$@I¾×ü?ïGΠ·p¿à^–%›Åï¿âž:Ãu`)¿×X
1/¼ AGNbcuNVSS J142750-321515?ï÷ŸÂèä¾?V7sBef?PÀz.6'u?V7sBe^?ïÉHŠª?'(ÿªb¡?{u[ûº«–?'(ÿªb¡?ïPáN"E×?‹Ù®›c?•ãÖ-—E:?‹Ù®›\?ï±ãÝX§Û?}nJŠYñ?ƒ‡©Ö	@?}nJŠYô3FGL J1427.9-4206@t6m
J@1Cƒ`r0ŸÀ6p`w	LÀ:€®n<ô}?þx"¹7Ē@ ·…gÞa@⾛ܔì¿ßRØȌ¿ãÙù·w·-¿ä±¤0Ëпç«)>gĵAGNFSRQPKS B1424-418?ïÙ=Í5o¼?rQ~X½]?saeH"p?rQ~X½^?ïà<B¶?xñW´?obýIï9?xñWµ?ìÙèÌGgì?¨ÎbƉu€?¹0¹ÄÀ£?¨ÎbƉu€?ïÿ¼¢,e?ÈM‰
?×tø¦ó¡?ÈM‰
q3FGL J1428.5+4240@S^<Ö_@P93À9KÏf@×À;>vƒêÛ¬À0‹áu%@W]ª*5‰?ù1¶@™MC?Ðm=ú¦=±¿ÐúMƒÁk¿á
a<…í?ÐLW
l¯AGNbllH 1426+428?ïò§2ö9?a'|ÈòÃ?[Ò±š‹)?a'|ÈòÆ?ïÙÇ!ÄÊâ?ƒI|b=F?soš1?ƒI|b=F?îÁ%S'¯ì?›]¦ù™6?£íªÍ…5?›]¦ù™6?ïÿÿ­(.>±Ó‹#I>œêZú/€ÿ>±Ó‹"ùÅ3FGL J1429.8-5910@s´à&Eå?õ ¿ÉÙþÀ7(g  ‰xÀ:zõ‹1÷Ê@wÿb÷*@ßaÏÓ½@†Ûw_ˆ¿Ñû@VÿŽ¿ãoÙU¶Ì¿èP]<•e¿ï	‡Q²>PSRPSRLAT PSR J1429-5911?3™žý‹
S?0/ÛÀW'?ïýŒÌ NŸ?0/ÛÀW?(Á¿5iqé?FGÇDT~‡?ïþsä©j?FGÇDT~‡?uý­³.R?eÖYzT§Y?ïÔz¤™¤?eÖYzT§]?*8·Ùà2?&7Ÿ«ƒÁO?ïþ\t'aý?&7Ÿ«ƒÁN3FGL J1434.1+4203@RÄøä@P^ÀW¦À:4ûŠOzÀ<'~Ê
{¿Ù–Zê%@m÷êï]@"í¨'Ú¿äÐX؉C‹¿ã%8~‡×¿æÖ&'¼¿çF£¦@y AGNfsrqB3 1432+422?ïú>…èÄ?Q­Þyȳ?Gè_€òØ?Q­ÞyȦ?ïǘ—ó?†F‰ÛX¸?|3ñ4t.?†F‰ÛX¶?ïwó'€2Š?ŒÆyßvUñ?'Ïù®Æ?ŒÆyßvUó?ïꁖMŒ?a$ÂKMð?e~i²såË?a$ÂKMð'3FGL J1434.6+6640@[a¿7¸Ô@G±K¹ëÀ:µ´ZæÀ;õãåî¿ð(¿1-Êi@
Rß3›Ž?øCú€º$ª?Ð¥zbò"†¿À»iÝ=â¿ÓIáùR¿Ç7Tºc±AGNbcu1RXS J143442.0+664031?ïîgaÏ?n§ÿ|ïõ%?a˜ž~€1e?n§ÿ|ïõ)?ï°LpP?**Ã	?ƒìãþ«Ü?**Ã	?î×äF81?˜€SÏV¬Ê?¢·ëœ|ë?˜€SÏV¬Ê?ïþ&ãìéH?+™ß]­>?-'Á1k?+™ß]­s3FGL J1434.6+1951@5`àЏÐ@PS ÒH7À:0qŒ4VIÀ;q°-YÕ^¿ùu¨6À[@RÆ ‹;@ûõƒ¥¿æj²Y¾¿æ×Îú_¾=¿Ó篧"Y¿êR êNqAGNfsrqOQ 253?ïøÞ¿Ÿ*S?Nmn($q?L…ƒV¯Ù?Nmn($a?ïËBé4?†"nLžÓ°?z^‹r|e‡?†"nLžÓ°?î¹}Xàjp?˜¯š|âÌ3?¤h*qùXÿ?˜¯š|âÌ3?ïýX;ÜÜÙ?D@Ê>ÃÚ`?5>!Mì?D@Ê>ÃÚD3FGL J1435.2+2023@6¬ ŸGX"@PV³`<ÎÀ9µc¾yåÀ;ByÙె¿ñõ[YBœ@
3oЍ@oU ›k¿çž3däå¿æè0-¿Û¡O–U¨¿ïÿ«mâgAGNbllTXS 1433+205?ïÞ¥o%Ñ?}àHn†¼?pó­Hmü?}àHn†¼?ïÍL‡žÏ?¨F1J.CN?œFVo&N?¨F1J.CN?ìû‰rãÎ?¤SŽJÑS?¸'ã´há‹?¤SŽJÑR?-¡Â?†!$½9ñ?€Ü—¾¹?†!$½9ó3FGL J1436.8+5639@Xp6ßû}º@K'ÿyÈÀ9÷ ·›`À;ì±AV¥?éÜ»¤¨¹@ïçÈ{¯N?ÿÂ\@©õ¿åëÌ´¿ãÈ|µLs¿Öf÷ŒO?j¿ÑPíè®ÞAGNbllRBS 1409?ïÙå,CZg?zÕý}-C?s
iÞRÌ?zÕý}-A?íù[¡DS?· oûן?°5"õۅk?· oûן?îãaKì?–`šØF|i?¡Ç.iëA2?–`šØF|j?èèm
õî??½N–ä­N?Ì^KÔ(G?½N–ä­N3FGL J1436.8+2322@=ÔW?ö@Pzd_ûéÀ9׎¢Å'FÀ;¸"lá«¿ÔxlÀ?9@ï¾v@B½ŸˆF
¿ä*Ic4¿ç-žÂ+Ø¿ãL:'K¹¿à§Á^&sAGNfsrqPKS B1434+235?ïÿ§J­A‡?7z~Ýd*?-T¯ž>ð?7z~Ýe	?ïÌ%¡u2á?…M£íoš~?yí/EfT?…M£íoš~?ïçÿ1ì+"?k*Røé²?hÎÔ{°?k*Røéµ?ïíþ…?]7i(€=?b€ïô{G?]7i(€=–3FGL J1438.7+3710@OÏ`?Û¸"@PQɀ2WÀ8¬N¡MÃÀ;¤ÖR5W?îÅ9oý@k0¥F@êÆ?iøA¿ã+ñÍ[¿æwè­0­Ð¿â'^³®\Ž¿ì÷=Ûû
AGNfsrqB2 1436+37B?ïú¦ã;èÕ?HHAôÿ0Û?Eds\©ü?HHAôÿ0Ø?ïØúV$Q?ºØˆJ¥?s'Ôí×~±?ºØˆJ¥?î÷KD¶ ì?"v羦Ñ? ‹K´ñ2?"v羦Ñ?ïúf3…ÙÉ?C8nõÝ]?Fg1è˜Û_?C8nõÝ?3FGL J1439.2+3931@Q2Ü¿ôw6@P²-LiÀ9ç:Þ"_¦À;Ÿt´*¿üBÊry]@Ѐ:øÏ_?üU«`@‡…?Ê^ɼ–ò¿Úä^ä¼ØŽ¿à†8<B·œ¿Ð›¦G"AGNbllPG 1437+398?ïö—Æ
Ò[?SE'µœ?RÐsä[K|?SE'µ§?ïÔpcÐ?"Ý8èd~?uóÇÎ7—ë?"Ý8èd?ïLŠb?"Zš8Y+;?œ¶n¼s¯ü?"Zš8Y+9?ïÿž¡ø;?ëqٖO?W¿ñÆ?ëqٕæ3FGL J1440.0-3955@tIñQç@2X&NyáÀ:MJ4¸À;¥÷T_Ó¥ÀrƒSÜöæ@
¨Ñò%¡Ð?ýÒ
ÿGv?ïZ–¼
6¿ëê%NÝÍj¿Ù#N§ƒ?R}!$#1AGNbcu1RXS J143949.8-395524?ïÿ-—³‡?!4Ø1ïò?ZM	Žó?!4Ø1ï¬?ïàŠ_où?x‹Ó¥*ÅL?ouð 9?x‹Ó¥*ÅO?ïªëÒ«g/?}2Æ)¯º?…EU&4T?}2Æ)¯º?ïÿõ=qJ>é¯%ÆÕè¼>ՅÛkç>é¯%ÆÕá²3FGL J1440.1+4955@UûÐÓ@M•ƒßóðþÀ9¹[O7À;ó¼w¯d?Õx æ³"@c0¦æß@Ð^à
AL¿çuµòžK8¿è®€9²d}¿å åõ"¿Ü+µ×NJAGNbllGB6 J1439+4958?ïꈉ?h×ðq#*ý?ew÷ïvá«?h×ðq#+?ï~>ûRO?¥éÚxæЫ?œp8 •¶?¥éÚxæЫ?ïE<m|ï?äñYúëÖ?—XrP~'3?äñYúëØ?í­¿¹)%4?¥½â¼	Y?²'6¶Öh?¥½â¼	Y3FGL J1440.2-1538@uÃ?…Q
@Cßcߣi&À9§%?TªÀ;ÔCéd?ÔGÈÛ?p@¤BQ3Na@¾@—õ«¿ÐÆqO3Ö¿étÖޕïb¿å _ƒÉ"É¿âÑ,¾'ÅAGNbllPKS 1437-153?ïûl{y`¾?E§0CU?BN}¬?E§0CU?ïv`² <D?•¿‡7ÜA?'3é«øwz?•¿‡7Ü@?îò"†4í?˜YQ,	ª­? ×·œ±/™?˜YQ,	ª©?ïi»ôW?Œs§‰½Ÿ?-òȁu-?Œs§‰½Ÿ3FGL J1440.4-3845@tR̟¶M@3ZŽà3·À9ÔuðG%XÀ;gš'Í¥:?±Â™¾¾¨X@Úf¸ñ£œ?û±^ûãç¿ïÏ	XU?æ[éö±Ö/¿ãè_ zù¿¥{1‹a·AGNbll1RXS J144037.4-384658?ïߟ3|v­?sh3ŠE¬?p0fAÄ©Ì?sh3ŠE®?ïÐPA~Á?€ó5fšXÆ?w×ß@Ÿoë?€ó5fšXÇ?ïq)]œ%5?Œû¸{Õì?'ÚÔL{YH?Œû¸{Õì?ﮉaµï³?€¯m˂¸?"]§'"B?€¯m˂¸3FGL J1440.9+0610@vq[«–ò@LKT´FÀ9<¦9»±À;–g¼§»›?á¦9xzBÅ@Ý¡ejè×@úEà4Ä¿æG®)ôp*¿åYø/|¿ßu`Ôí¿Ø–Lgâ'\AGNbllPMN J1440+0610?ïÿÀŽÙÃ+>úóKX4ŸÔ>ÿ¸"jÅ>úóKX4œ¾?ï²ê‹x?	¾§_?ƒ¾…]!¶?	¾§`?ïÍS&•Õ?z°¥Õw.?yVlµw"Ô?z°¥Õw4?﬽…Ö?wŸ›?"й¹žŠ°?wŸ›3FGL J1441.5-5955c@sÅ>€8Ÿ"?¨{϶ŸQÀ8j3àØŒÀ:5é$h;?ñâãd"Ó@…ÝÞÂî}@x*.¤¿á£º"ˬ;¿ß_[61•¿áû Ôvd¿ç/z¬nˆtOTHERspp$?ÂáL5åÚ?ç:)µu?ëG¬ò¸†‰?ç:)µu?Ì®¤µÜ–º?Ì£^Öoi?èÔV҈ÚR?Ì£^Öoi?Ú¨®3–Z¬?¹£*é¿…?⫨æ4Òª?¹£*é¿…?ܔñg-?ÀXºÑuÛ?áµý‡Liu?ÀXºÑuÛ3FGL J1442.0+4348@SC8€®@Oû¿ÿ^ðÀ:R@|ÇÑ»À;سc$"?ìȨƒu@
µ2g±??üyvèÀ¿íÖÚâå?¼Ñt|S¸¿­).ˆª¿ÝØÓ+ò³MAGNbllSDSS J144207.15+434836.6?ïÚtêPA?u¨h'?rÅÀ
×ß?u¨h'?ïG2Ó¢V9? 4–1 ¸Þ?—¥‹µ8Ü? 4–1 ¸Þ?î¥cn©@±?™¤ÍÀ'•Ÿ?¥©Ékôü?™¤ÍÀ'•ž?ìzõýà W?°Íšl'nß?¼(PúýK?°Íšl'nß3FGL J1442.6+5156@V· '½´@LÌûÆnåÀ:ÙPÑÑÀ<™‡ûâd?åG»ÞgÿÄ@
q¯ 5w?þ–?ïX¿ïýÓٗœ¥?ïÂpdÞÁ¿ÐͰý뚿ê8Te†(AGNrdg3C 303?å¹q¯!?ÐH¤´«d]?ԍðÞ¡½?ÐH¤´«d]?á+ýñ`Wƒ?Ó³L;¾ÿ÷?ݨ?Pû?Ó³L;¾ÿ÷?éA-"'µI?¹f‰(`H?ÊûI³a*Ú?¹f‰(`I?åè"tü"Ó?Åx|–Ô?Ô.ÙÖZ?Åx|–Ô3FGL J1442.8+1200@ ¸G '¨;@MéšÑVŸÀ9±Ú/‹ÞÆÀ;|1u¿ãy:M¦ƒ@^ŠPPzl?üºlà¨÷°¿çyqcªÌ¿ÛvI³ç¿Ä\qî¸b¿Ý¼ü'.¸AGNbll1ES 1440+122?ïû)Qbt"?BéPþ-Ž?CZºv/u´?BéPþ-œ?ﺇüñ?Œx©¿*}?^=ûC²?Œx©¿*}?ïª|ŠÎÞ²?€¤\¸?…`ÝLHS'?€¤\¸?ïö,…Hšß?Vƒè.3à?S¦õnÊD?Vƒè.3î3FGL J1443.9+2502@AKy@]¾!@P,rßñl¿À9D–¸=ɏÀ;š÷Ÿnd¿â/	Ì@ø¯.+aƒ@V¾|'¿àEËE…'ž¿æ(>Yú?¿Ô!Ë4yã¿èKŽÿaÊAGNfsrqPKS 1441+25?ïû%oô‹?Kž¬éÎç?CkŽ@-Ô?Kž¬éÎã?ïj]/B?¨ÖÛ߆?2´Z¾$?¨ÖÛ߆?îªDÂMÁf?—"ˆ\B›ƒ?¥[³Û#é©?—"ˆ\B›'?tË/A?´§AؔË?ŽU"Í4/Â?´§AؔË3FGL J1444.0-3907@tZàP7P@2¸ßh°ÄÀ7ó¢²G‰À:¶³žþ]i?ñß°	´A@æˆ*?üùë`á—4¿ÞAPb#¿ÖNÏA­Z¨¿×`·-†Ô¿ÙÚX³5€AGNbllPKS 1440-389?í5mÜ~[?²VZ–¼×?¶T—
+?²VZ–¼Ö?í8bÜ?³ô;/Ì#û?°ƒ®<é"?³ô;/Ì#û?ëY¨¹ã?­-ƒßøH?ú›™]q?­-ƒßøJ?ãZ®¢_?¹†¿:)c?ÙJ£È»AÐ?¹†¿:)c3FGL J1445.0-0328@uÓ1ŸŒ¨@HuËCòžÀ9§ËtÝøÀ;p	{¸¿îÚœ"ê@,"+ž>o?ÿIØÿ5)Ø¿á,š¾ÃÛÉ¿Ù0õÿ~®d¿áºì¶)м¿ÖæÏ7—OAGNbllRBS 1424?ïíšMÂÌ?eßÛÎ	¦?be²~=4€?eßÛÎ	¦?ï°^xV"?'Ž"­"¤Ü?ƒèaêwX±?'Ž"­"¤Û?ïAË•Qx?'Y¥µés¹?—ƝmUÑ?'Y¥µésº?ïúñ™tF?GpÞÂxµ?D9Áš.åA?GpÞÂxÁ3FGL J1446.1-1628@u,ù jn3@C$CÀI0ËÀ9á·äkOÀ;†­âü¹ú¿ìùËVÒ@¾…Mi@ßy_'a¿èA5Ø)!¿ã†È1:=F¿âÛåÍ¿æªÔͦ^AGNbllPKS B1443-162?ï÷á†åø?WñÜ`þ?P<óø4a?WñÜa?ï°ƒËp?Šà÷óx=?ƒø|ß
#Î?Šà÷óx=?ïqѯ›?Š¢äíð?'ÜÅÊŸï?Š¢äíø?ïíÄå,<h?bë R¥7Y?b;Ó×½?bë R¥7]3FGL J1446.6-4701@t(Óõ¶@&ÓÈß'·À9äþú2À;]Ê÷àvÎ?ïû¶' µ@xߥA˜|@bÏߦÄ%¿ê Ð]â¡¿Ô+ÿÊrvâ¿äg=› ¿ïþ¤&Kª_PSRPSRPSR J1446-4701@?Ý#×iM–?Ì å÷=–?ánKY4À?Ì å÷=–?Öñ"FX!Ä?Ðr0¥˜(?ä‡5ÜÓï?Ðr0¥˜(?ßm<ñöŸ<?¸/¼¸ÜÂ?àIa‡°b?¸/¼¸ÜÂ?ÔéÃ2øß?²ØBº?å‹žfƒ?²ØBº3FGL J1446.8-1831@u••:@B:)@k*À:q?8$4À;›Ÿç't1?ãU4%‡µ'@
¯–§w?û'#¾Ì#?߬$Éì{F¿ï'Hˇ
·?î¦ïc"¿Ó±²ÚÞ2{AGNbcuNVSS J144644-182922?ïùâ×<²Y?Q–÷ó´ví?Ht£
6žJ?Q–÷ó´vö?六AåŽ?™u×^cº«?†¯†¹Ûÿ?™u×^cº«?ïoÉ{{+'?ˆ_0Ä
V?'Аš·?ˆ_0Ä
T?ïµcö*-?˜–F©Å˜ä?'¸çuu?˜–F©Å˜ä3FGL J1448.0+3608@N"ˆ?Õ%@OÛ¿[o'À8߉çtî¿À;;Ɨ(¦?Ø9scÏÞ$@×vôÓý?ý%ßbц¿Öã"8'þf¿Ùïw`x‡¿ÙAúÚ.è©¿ÕñÆOÖAGNbllRBS 1432?ïü¯ØæM?D^!l¤Sx??8͕ó?D^!l¤So?ïÉÓåÃ?‡eå⚥Å?{}p–
'?‡eå⚥Æ?€ö8–?4©e??‹'ŸÂqÚ@?4©e??ïΉÇ6v?p•Fó2}?x»dùě?p•Fó2~3FGL J1450.4+0911@ lŸædÎ@LUÁ HàDÀ9íþu¼D¿À;»˜õ.릿éFïþ€#@
Ç+Î@ʽ`s2R¿æ°²ë$P¿ßt ×·¢¿Þ}®±Ù¬Y¿ì6ʸ(-¤AGNfsrqTXS 1448+093?ïrlÓ0‡°?•uî0?'²e™ï	ä?•uî0?ï¼Vµô[m?‹ï£õËs?€êR'é$œ?‹ï£õËr?í•'f7B?§7–ªiÊz?·ƒSìÎEî?§7–ªiÊ|?ïøzçŽþ?M`ôšF¾?NaÇà	I?M`ôšFÄ3FGL J1450.9+5200@VGŸõÔ-@LF{ÓöÀ9Á
Ìq]:À;¿bÀ¿xP?ða#""@7_a@k=ŸrÌ{?ïåq Ã^¿æ>Ölá¿à.Έ°=¿èŒÚWéÀAGNbllSDSS J145059.99+520111.7?ïfNo¿a?"Ī3/4?¦ld'¡?"Ī3/5?âv@þã£.?Ð~P0Y›þ?Û~8¹£?Ð~P0Y›þ?鈶Ö]Õ ?²Ù\´¡é‡?ÉÝ$¦ˆ«?²Ù\´¡é‡?Ú$4RaŸô?¾U¨´Øæ?âíåÖÏ0?¾U¨´Øå3FGL J1451.2+6355@Yæœýç!@H;ô|ôÀ:ÌVô›¼À<,SÐa¬Ã?Ï+$]¤Ã;@ÿ˜_ݶ)?þ°Á(~Ï¿í‡t[¥ ¿ÅíF挎¿ä¶ˆî¦'¿ÎùƒÆëÙ¥AGNbllRX J1451.4+6354?ïµ¾¡uE?±Y¸Á
ΐ?	H+ÑW"?±Y¸Á
ΐ?îZ'Õ!?¸… 9dÓ?ªVãÆ­î9?¸… 9dÓ?íÒD"ŒÎ?°_SøùY?·¹mÛۙ"?°_SøùY?îÀÖgÏÑ?¦·W¥*̇?®ò™ƒà?¦·W¥*̈3FGL J1454.0+1622@2Œqà,l@MÖû¿ÿ^ðÀ9øNz·VCÀ;ÊmÍÓ?¢]‰3ue@@ם¶3Ù@¿‰ÿ¯~¿ä!¶"F摿螓è:ø‹¿äNþC^Ç¿ïÿïÛ*ï©AGNfsrqCLASS J1454+1623?ïüô®ëø?A¤¡Xší?8Zˆ¡â9Ð?A¤¡Xšë?îÜý[N`?¥®ñav?¢0*Ní?¥®ñav?ï3È_w?ã·CûYä?™†ôÝ?ã·CûYã?îdX (Îk?œmqç1/?©º}ýsA?œmqç1.3FGL J1454.2-3751@t'Ž wm@2ìïÔ;VÀ9R¤ÅFƎÀ;qÆ:âT¿ò7wÀÖÊR@ks]oǹ@ Û´¿ç6üºavy¿è×{È´uy¿îs€Wÿ}¿ÉYSæ(ŠÛAGNfsrqPKS 1451-375?ïûÎæyò*?H›ÌWä?@Äf7[?H›ÌWï?ïᴟ×¯?y¸émӏ?nK`p(Q'?y¸émÓŽ?ï@oðOä·?Àœ<O–?—òöi?Àœ<O•?ïüÊ:/c?;©/Áïà?9®."ã'?;©/ÁïÛ3FGL J1454.5+5124@Uêx $Î@L9o¿«|À8W!CF¦­À;IŸß-øa?ð¶zӅΌ@»W";Œ@«¯‰øè¿ße5x÷|¿âBÿ÷æ¿áï'Á;§ª¿áì6CmAGNbllTXS 1452+516?ïþïÏH7?#ø]$AN6?!~Š‰?#ø]$AN?ï`Cλj?š§È¾Ë¹j?"÷†(ŸÒÂ?š§È¾Ë¹i?ï(Ú§ñª ?"ø‰Ž¯±!?šä«'?"ø‰Ž¯±!?ííŠä?¥ÿDgzÕâ?·h"¯ðß<?¥ÿDgzÕâ3FGL J1457.4-3539@tž5 ÝD@4‰4ŸCý†À7he²â?üÀ:ç·I­Èü?úMÔ§6»(@D}Ä&
+@\'eîqb¿à
´5Òñ¿å'Úák
¿äã\C«Y¿è'Ÿ5ÁOAGNFSRQPKS 1454-354?ïøÉüŠïv?MÝvÒñŸ?LØ
ÔB$F?MÝvÒñº?ï٘EË;?€•UI=1–?s3Ý1bÆ?€•UI=1–?î´Ü‹Œ˜
?™6›_摲?¤²7G6K?™6›_摳?ïÿr:rd?—.1ë?¸½Ñ³v1?—.1ë 3FGL J1458.7+3719@Në<¿£ï^@N°q?Þ<aÀ: –Ϻ¾À<DðÊØ׿È$=Æxä‡@¨ÜRPÚ¹@êvjG¿äé¯z<Ã;¿äiÏ°""¿çñԇðé¿Ûœ–½àåwAGNbllB3 1456+375?ï÷ØÝ7?aHø$é¾?PxÎEϓ»?aHø$éÄ?pš?"²ç;s%'?‰|cúY£?"²ç;s%"?îÐѨ×÷=?š^Byu¨?¢òår€Œ7?š^Byu¨?ï­vÅWG?{ñ,'¸º?"¹"Nª.$?{ñ,'¸»3FGL J1459.4-6053@sÞ
?‰'Ë¿üƌ µ,GÀ6íF4—·AÀ9ûÏÑdB@hzn±@
E\-}@¥€
¿Ý¹›¿änì
Än¿çÿP§Ë¿î¶œxŠðPSRPSRLAT PSR J1459-6053?¿åäGµŒ?õÖ!1?ïÿ¡hná?õÖ!2?%¯ÕF``?C›ó_â?ïþ¥«š?C›ó_ã?ƒŒÝ­=! ?~%Œ,ú÷Ì?ï±Ì‰K{?~%Œ,ú÷Î?*³Ì… Í?%ôµÐl?ïþVôÃ7¦?%ôµÐl3FGL J1500.6+4750@TGŽÿâ£Ï@L¸®Ú«³À9þÁqN÷µÀ;t7.jv–¿çVjòß}v@ }kœÆ@$ q¿ëŒ$œJ+¦¿ßL©_Fë¿éù"€­ºc¿åø"–ðAGNbllTXS 1459+480?ï'Î
UF??—y¯NNj?‹L}j®pÄ?—y¯NNl?ï•a¼þ¥?"²BL=ws?Š¹çÀW"?"²BL=wr?îÕʔ?¡ðd'¼‡?¯r¯ÃV¾Í?¡ðd'¼‡?ïÔúóªH?r¦?ڞ¼û?u'†}*Üu?r¦?ڞ¼÷3FGL J1500.9+2238@?pc_Jé2@N.µÀ@ÍPÀ8î÷Œ"÷™À;N;õy"A¿åŠ<ïÊ}½@é×µM?þ±J b5ª¿à'Ì!ÅçD¿Øz"ZóÁƒ¿àørOu¿ÕÓËÕzWAGNbllMS 1458.8+2249?ïÿ'–?QµÐ?½9š{*m?Qµ—?ïѧµDo©?†‹`ˆL?w,%]È+,?†‹`ˆL?ﺇfÆÔ?€­/·¡ZŸ?^&NJÿÝ?€­/·¡ZŸ?ïÿiɱu¨?=¿Ù´òÌ?ÆÉÑK0¯?=¿Ù´ò13FGL J1503.7+4759@T;[À6ã@LvÊàc'†À9ƀÈè;¾À;›)гâ¿Ø¶á´'@ç÷ˆã@½è@EÀT¿Úªüg´¿å>¶DRÈØ¿ä—$äæÊ¿åŸGïêAGNbllSDSS J150347.99+475930.9?ïýK
7ÿc?7(¬)Þ]?5§–@ð¿?7(¬)Þs?ï´è§šNð?‰|DL!l?'ÅÖlCþ?‰|DL!l?ï>ñ3\?'±¢úۍu?˜!ßy"|©?'±¢úۍv?ïߚºáq^?fw'8¤©?p2¢GQ@?fw'8¤«3FGL J1503.7-6426@sɛ€#¦ÎÀ–šÀ
F«À8å¢4rÎÀ;vJßø#?Û毶UUâ@­êY$´j@¦¬ l¿àjÞ|ô|¿ç«
ü÷ü•¿âÄjMÚ1¿éEpÑ4¡®AGNbcuAT20G J150350-642539?ïðAܗ'?b™¦`zÃ?_|FÐûξ?b™¦`zÃ?íó¿¥x!­?¹´æŽVØ?°bÔ>ò›?¹´æŽVØ?î·0j\o€?›ôŸyÌ	?¤ŒùZ9ÿ?›ôŸyÌ?îÑfÍîçS?sßŠ<}?¢é"!ŠÐ?sßŠ<}3FGL J1503.7-1540@u|0¸,,@B?ñ7À9&M±cººÀ;*"ž­Õ'Àý¸à[Ê×@¡nu©z?üPOÞº‹¿àü᫽CÔ¿æóEkˆÓè?©Ÿº"®´<¿Îs0õÒeÏAGNbllRBS 1457?ïüœ'ð'U?>¿ÒÕϸ?;h{m_·?>¿ÒÕÏÚ?ïÖѱZqª?ôëV3O?t—'RÇ*ô?ôëV3M?ï—Ô¢#¬'?‡xdSÔ'?Š
×wÛð?‡xdSÔ'?ïÿÿÔb±$>šdÉYƒoš>uΧn!=>šdÉYƒ³3FGL J1504.4+1029@&Û`C6¶@KJ0 Y;ÛÀ6"bÕ¸-ÙÀ:¨
ހ@ÀY#²·£@"så!Wh@;l0ªÂ·¿àŽ™ë4¿äˆpeSýê¿åRԐæl±¿éDŸ¶š©AGNFSRQPKS 1502+106?ïx®Õ¼?šL"ÔXð?ÿ*%_hŠ?šL"ÔXï?ïʶê6Ï?‡#•Xõ^?z¤Šäð˜Þ?‡#•Xõ^?ëÿ€	?°Ê¯Z\2?ÃëèõÿÞ?°Ê¯Z\2?ïÿúS9ùô>ÜáŽvNƬ>Ƴ1æ.>ÜáŽvNÅ3FGL J1504.5-8242@s3Y'ÿÀ4øc ¹HŒÀ:WG6wÀ;·^j¢Ž¿èìãuÃ@Í)éÞV@aÿ ^¯¹¿é³· s[¿åqµ%ªù,¿äÄÖô~E¿å/Ë6õŠ†AGNbcu1RXS J150537.1-824233?ïïc‡´?gM	RÒ+?`œxðáJt?gM	RÒ0?ïÕTFêÂ?'M¿Ìí?Ö?uvÕ܊žþ?'M¿Ìí?Õ?ï= èÇØ«?'†š½ìõ?˜KâçêÂ?'†š½ìó?ïòjÕ}à?XqÀn¨û?[*U?Á4?XqÀn©3FGL J1505.0-3432@t¾¬à2Û@4³	¿œb¢À9­&|k‹iÀ;ÞŽ–0Y?ᜏ Ï÷@ ƒ™:@×ýFKê¿èäÜJÚ$*Œ¡—¿ä?[ ˜D
¿ä]cMWKÁAGNbllPMN J1505-3432?ï~Ý7­w?"%њ–­?ˆ H²¢F?"%њ–®?ïtv
'Øi?–Õì؞…?'q>»òã?–Õì؞…?î†@E,C?Ÿ¨±%>?§›û¯
;¿?Ÿ¨±%<?íGB&ñ¹¬?7šs¥w?µÅîÈr2š?7šs¥w3FGL J1505.1+0326@ä×?Âb¼@I ÷þ½áÀ8…,$K9À;p§I……?Ò	®³@4؉™q@ßú D®†¿å6}âÑ=¿éÿHÂ^¿è иØ$¿æI̧¸ìAGNnlsy1PKS 1502+036?ï¥lþrÁ?Šu!ò74"?†¤ÀcOŸÔ?Šu!ò74'?ëžaÈ5 ?ÆåÂ-ªá?Ãņxß)?ÆåÂ-ªá?í¿"³2ÁÈ?¡8¬ˆ 8?²Úfiñ·?¡8¬ˆ 8?æåRó.Ȗ?¾Ã(aSsú?Ò5Z¢nÔ?¾Ã(aSsú3FGL J1506.1+3728@NÉÍ_™Ã‹@Mò•¿ðExÀ9C×xø9À;É}»Ûä?ò]§rö@"äÀ`Ù@Ÿ+À£Ò¿áõpÙ˧£¿æ.5Lèæß¿è«øP€˜c¿ïü8—Ô¦AGNfsrqB2 1504+37?ïïYqëIõ?g`RyHm?`¦Ž¶¨?g`RyHk?î7»¬8?¯P¶a•ÌÕ?¯Öü"E<†?¯P¶a•ÌÕ?î|&fþ¾?ž€SO‹õ?¨>홐%?ž€SO‹ø?èäb	¡£"?´‹u^4	?ÌnwÙyqð?´‹u^4	3FGL J1506.3+4332@R>Dàá6@M#˜ÀUÆÀ:ŒÅ½äÒ}À;ý¬Y¾O?ËV‰?•}f@
Òæ6«7Ò?ÿ'T€	û?ïð·EçÒ¿Ï"ÑžâH¿Þˆž«Ò+¿â)˜'©AGNbllNVSS J150617+433413?ï"tr¼ü?•/É8Ú?ŠâãPþA#?•/É8Ú?îëTóNß?§ÚæÈ÷Šø?¡J°Î{?§ÚæÈ÷Šø?î|½ñº,? JŒÓ±`0?¨4 ä_ÝD? JŒÓ±`/?î8€¿´?£†
Mͯ(?¬wçôÈ?£†
Mͯ'3FGL J1506.6+0811@!VèË@JiÙÁfgÀ9µ/V/À;€«rßñm?ëNÜ~h@;=‰ù=™?ýûö€¥Vç?ÅUw…úù¿àŸKã`놿Ϯ"ý¾¿àÿ{τ7AGNbllPMN J1506+0814?ït)ØRû?–<@«´&?'|ZÄõ z?–<@«´&?îËVÆß?§"l	ð,?£J"ž~'?§"l	ð,?îxFè¯D$?š+<€#­?¨{'u½·?š+<€#«?ëí¸k"7•?­ ·j¾™á?ÀISw!­?­ ·j¾™á3FGL J1507.4+1725@6ëòÿf}
@L—«ßí;À:—'ï2RcÀ;Ñ<*R¹á?áËÌVÛ.@«¤íµ¥"?ü‰!ACAH¿ïê(¯k?ïšÐsÓê׿Òî0÷wN¿Ób¡éAGNbllNVSS J150716+172103?ïù`Ù3aÇ?TΨ
Ql?J|›2xäŠ?TΨ
Ql?ï–(C˜þ ?•!ü¼¨
?ŠuïÀX?•!ü¼¨?ï~ ï%U·?ˆ[ïs	Ûâ?+âUI%?ˆ[ïs	Ûà?ïQ'E<q?'í¼Ø6l?•Û
÷XqÐ?'í¼Ø6l3FGL J1507.6-3710@t®ÿÀ	oë@2-×,uªÀ:	JÅöï¶À;Ÿ{Òuð?Ì1kKÂ:@
«$õØ´¸@jßÇÑ:?ºWZ€Dl¿åH¡y·Ñé¿ÕT…ࡍ¿æ…ÛÊý¥ïAGNbcuNVSS J150720-370903?ïæ­7y ·?u,¼#||Ë?iRȆ_GT?u,¼#||Ì?ï|ɖÃà·?—œßLòTC?fÍ'ƒé)?—œßLòTB?ïR8ä8œT?¶¯Ælã¨?•¸ãxìuT?¶¯Ælã®?îcm« ??™ÿhÀÊ+0?©É%Eþ¼?™ÿhÀÊ+13FGL J1508.6+2709@D€"ð½@MÈ÷`MÉÀ:YÞ9ÛÀ;³¤ës¸¿ÐŽïnYÇ>@
2ôU¿?ûXt@Éп圏º•¿âj­…+Dõ¿ÅÌò—mx¿Îå}éÃ[AGNbllRBS 1467?ïû÷Z=å?KúJ9ÁR/?@"—ˆm×?KúJ9ÁR)?ï·ÔÊ®"P?‰™r'$]?'
ÍT^ëÆ?‰™r'$]?ïhìÌs8;?†~}µ"?'âfq˜øÅ?†~}µ"?ïèŸWo?dJXˇù?g`¨€í;?dJXˇø3FGL J1508.7-4956@tF7GMœ@†¿ë½ÔÀ8¥ïm
ÅVÀ:ô"Ýz™ú?ã;Rø¸@C4LbÚ@Ø!¿˜[׿çßsâ3¡¿é÷ž€f˿筕~g1¿èœpc•QAGNbcuPMN J1508-4953?ïöoÏï¦T?VJ-軕o?S ` ³Xñ?VJ-軕p?ïUNèú2…?©¦äêa?•V"๯€?©¦äêa?î°öÀ¼? š"V?¨ÿ"ô>? š"V?îC_sà&?"};£éka?«ÎÊÁý‰?"};£éka3FGL J1509.4-5850@sÿ?á—_¿ãÄ&½ò·À6ÿ\£oqÀ9ê÷ãÑÌ@äª1xg@¶'ž?ý˕/&´?»Í}þ'¿ß!]
ÞK6¿äÀj4À벿옗A‹Ì¹PSRPSRPSR J1509-5850?1ÝF_˸¬?(|_F$Í?ïýÄW4‰?(|_F$Í?/ÕYÚ0?Hð÷X¹?ïþòªoâ?Hð÷Xº?sÇïT˜ao?aLž¨±
?ïØp!VÏ>?aLž¨°ø?a2=ô›kK?ZÍ;« ?ïîÍÂd•?ZÍ;« 3FGL J1509.7+5556@Võ: !Þw@Jߥ¥À9ðE;ss•À;ÉZÆõó7¿¡›÷êH7ñ@¬‹ä¥0§?ýí2?î,™¿Ó»6.\¬ ¿ß&ŸêŸ#O¿ÙÌ4mè2P¿ÏÞÇ}À AGNbllSBS 1508+561?ïö¢.nÍ8?X˜™ÙìÌ?R»£"eñ?X˜™ÙìÊ?暴!ď?"éd@6Þ¯?…ÿwŽÜ~?"éd@6Þ¯?ïCõ‰¥|a?"qÕR¨Ò?—NËPsä?"qÕR¨Ò?ïîF´23?ZY«®Z2Š?a¹KÍbÍk?ZY«®Z2‰3FGL J1509.9-2951@tù_™Ã‹@8F߸aÜÀ9›Ý÷vÅÀ;|4*©÷¶?îRJ|ÈIþ@ úô¨^@@âf'†¿é
7a|X¿ëኃ›¿áeEy±Ç¹¿ïýl*±À"AGNbcuTXS 1507-296?îÙVఀT?¢3›cܨ?¢j'ô÷úÀ?¢3›cÜ©?æƒdù#%n?Íp)ºÇC??Òù6
¹µ'?Íp)ºÇC??붱•;?°!Ÿ9ŒÁº?Ãá%9«Ž?°!Ÿ9ŒÁº?ÕòÃ%þ£?¾U:gi9?åóm¯?¾U:gi93FGL J1510.9-0542@vÿÅG@EvÖ@†À8VGõbÀ:õÇþ0òç?íÎû?0å@<k~ÿ@gŽß×@™¿àp‹Ð¦¿æm¡v»P׿æ›\2ÂZ¿è‰.NjâAGNfsrqPKS 1508-05?åX;»"×ü?Ê£")RéQ?ÕOˆ‰ºP?Ê£")RéQ?â`J5GÒ`?Ð	˜<¼§p?Û?k•p[??Ð	˜<¼§q?å#ì"
?·@:f?Õ¸'»ëÓÑ?·@:f?ЩB'Œ-"?±[àã3³?ç«^·9é7?±[àã3³3FGL J1511.8-0513@v)ä p¸Ð@Epà<ìÀ9F ²'/À;.¥öŸ..¿˜p'Á]O@ãRi.lÐ@EÊ`‹Ûì¿ê½€i¥h¸¿ÜüD£aÞ¿×â†G'K¿á8;ÝÉÕAGNbcuNVSS J151148-051345?ï吔Æ!û?q
¾
ã?jok9ÞJ?q
¾
à?ïL{rùÛ?™Ù°7=œ-?–p' Þä‹?™Ù°7=œ+?ïgå­ñ×?‹ÒáÈ«ø/?"J_Å$?‹ÒáÈ«ø.?ï<ªOšHô?'uù{m?˜j¶¶á­?'uù{m3FGL J1512.2+0202@¤r¿#N@Gý}æOUÀ8zFgÃ]¸À;@¾61u?æ{S¨)Õ@ÌZÁ¶%@™ã KO	¿á½-'³N¿ã'÷­ßT¿â[eé#¿ã†Õ½à:AGNfsrqPKS 1509+022?ïòé덵¸?så%TëÅ?Z,(䔑t?så%TëÊ?ìSƏIÚk?ÁsÄÀõi«?½a˅±,¥?ÁsÄÀõi«?ïð‰Âñ»?"+—H	rÉ?œáîǡȂ?"+—H	rÉ?çãU@Ò&?¶w°ë&Ø\?Ð9Ué~[µ?¶w°ë&Ø\3FGL J1512.2-2255@uH^`=Wy@=xœ \–ÚÀ9â¾÷!À;d-–;@H?«†9¸¯õ¬@
®µëÓ?þôÿÆÊ)?ïËuȕ@Ö¿åïÿµ_ü¿Õ"'
»¿Û&ón¢AGNbcu1RXS J151213.1-225515?ïü'¶L(˜?@žÏs‹P?>ÂMž»8Q?@žÏs‹7?ïÁ³wŒæ?"E÷½™›?&D19?"E÷½™›?ïsQ㥽Ð?‰BuÑðH@?'•Ã‹HEÐ?‰BuÑðHD?ï+9i¢?":÷vô?Œ51¥—z.?":÷vô3FGL J1512.3+8005@\ýÃ?…Q
@A†ªšêÒÀ:›Ò‰¥/ÐÀ<*y®AÇK¿'&†ç
@Œj€ý@ˆ@ò`…%ï¿ë¥ìp¿äø,"¿ã'l"	ì¿ã3-ÇcZAGNbcu1RXS J151026.3+795946?ïøÙ)©Ï?[QsÜFã?L›¯YXÇÆ?[QsÜFÖ?ï¯41ˆÑ?‹xóûîÐH?"2óË¿5?‹xóûîÐH?îP×$¹ë?«Cb¹}¯?ªò´gV?«Cb¹}°?ï¼ipI(?yW㝰«´?€å£íµÿÈ?yW㝰«³3FGL J1512.8-0906@uôŸ`—Ì@D?ßéàÀ5nV·œ¹àÀ:¬²{ï@_"͊aî@"$åg£R@" ¿M¿âR´ü²©Ç¿æPH	"
@¿æ—/˜¿è4š7½ö4AGNFSRQPKS 1510-08?í
ވ>?»<ڗâU¥?·—¾>?»<ڗâU¥?ï¼	;2?ì—p6¦ø?€ý±3:Ù?ì—p6¦ø?êÇêøs…?°òSV¡Ê?ÄàT¦1å?°òSV¡Ë?ïÿý!Ϥ©>ÑZi ó'Œ>¶ñ'Ú·Üÿ>ÑZi ó&Ô3FGL J1513.1-1014@uåóà7Ý@CžŠÿ¢âîÀ91#ã4À:¨Â<Pg¿Ý¤}6Ñ<7@.ëBƒ³(@ƒ@;ÚL¿çÄëçf£o¿ê‡a(¿åõ—1´6¿ïý°<÷'AGNfsrqPKS 1511-100?í@U¼Ë?½0ZŸ}­?·/MýR¤?½0ZŸ}¬?îÑÝöì<K?¨lÝ'r ?¢â '<;L?¨lÝ'r ?耹˜½¸«?°qŒŸvÞ6?Íý	W?°qŒŸvÞ6?î/ãµñ?¤î‡ð€	?§-ÑÄ â?¤î‡ð€3FGL J1513.4-2549@u-ÿ¼ä!@:÷_f—åÀ9®P(6ïÀ;¦¨ñü1>?ùX,)(ÃC@GõM?ôò¬O©¶r?ÎÕÐxö-¿ÞB1õÁÛ¿éÝk±åüÛ¿éVcCÇ*!PSRpsrPSR J1513-25?™	êÅÙô?«¿I'ì:?ï7°¯qÑ1?«¿I'ì;?°u`BI?½#™÷Æ
?íüÑS÷½÷?½#™÷Æ
?Ä<Õ÷R I?·-Nº€‰j?êðʂ+Wî?·-Nº€‰j?­K¨ðY|?Ÿ,¿w·?\?î+EpþJi?Ÿ,¿w·?\3FGL J1513.5-3233@têµ_þmY@5këß·‹À8úaPÀ;[ƒäün{?ò¬»y"@ÃæÄŗN@¹áÀ¤ËQ¿ßn [·ƒ1¿æ:À&4Œ¿æ×G<Tš¿èœÉ@j:AGNfsrqPKS 1510-324?ïø,)&â?L!'«2֏?OOŸ[dt§?L!'«2Öm?ïÝ
Ì(åG?{ÌRk2pÀ?qyë\¹?{ÌRk2pÀ?îg†"Ϗ?™nzÓW?©‡Ó2?™nzÓX?ïá¨=6-;?cæ[¯3{ý?nWÂÉÒÅ]?cæ[¯3{ü3FGL J1514.1+2940@GÒtw@MQ™?׆dÀ:/àÇU"‡À;­ä9ÐÜ&¿Ý"žfC<&@w€*@Þ§ªÿ¿éªASv8…¿ìLû^ÿغ±Úá–¿æ3ɖ¿þAGNfsrqMG2 J151421+2930?ïÿä	%¨>ïÅ«W(ð>ëçöÚX¥ï>ïÅ«W(í|?ﮋؕé?ŽÊ^~BÏ?"~Ý	څb?ŽÊ^~BÏ?ïÔ°øÙ?u›H¸tëh?u§ƒð"p¯?u›H¸tëp?ïô䥜-£?Q.'5c/?V6´Ç¤»l?Q.'5c3FGL J1514.2-4947@tS°€0<@6™_·ö|À7ßÇËÜÀ:à)q'@å[½•ø@±aˆŸ?üûòª,¿ÓÛ'~Z¿×Š
oª1í¿á"Á0¿îö¿ëhdj/@,PSRPSRPSR J1514-4946?a·ÚÛtZ?\F6ͪ?ïîH%$ãŒ?\F6ͪ?p=þV°uô?'¥ÌJ·åD?ï߄RŸ?'¥ÌJ·åD?ƒ®%ÞfÂ?ɟü7Ô?ï±Gh†e¾?ɟü7Ö?H¤[²ˆá¦?=É®ó(j?ïùÖé]È?=É®ó(j3FGL J1514.5-4750@tdñà'Œ7@ Þ#ê¬À8ÅÅ.î*À;-R,¾?ãË4ôJât@àjR¯$p@£q ?[¿åݕH•ßÀ¿ä­8Íw¿àõ6â%Šº¿ëF'9LAGNfsrqPMN J1514-4748?ïéó'ñ]?e )¾Ù6®?f}ó¢–?e )¾Ù6­?ï!VôÖ?§û¬
#@9?›ßµ!e?u?§û¬
#@9?ìíQÁ¯yà?§Í(•çê?¸•qò"1?§Í(•çê?îWëó±q?—urùâæh?ª@Äèî›?—urùâæh3FGL J1514.8+4446@R‹UŸÚ%{@L7W`9%»À9J\OÝÀ;ÊÅ-œ}?íúgPàÜé@ÐîÕÒ°@¶G_eY¿àa·ã[¯~¿å"ÐèBþ¿å™‡¿Á¿ëU'Ö¢}]AGNfsrqNVSS J151436+445003?íÑÄsE4Ò?±CAÖª<³?±qÜeÖYh?±CAÖª<³?çc.߂®?ÇÜ(éÒrw?ÑÅ9¢@ú£?ÇÜ(éÒrw?阤€Ý?³y¬Ä…ô?ʝmü‰ý?³y¬Ä…õ?àkq¥IŒð?¸¶•"}Ë?ß)µlæ ?¸¶•"}Ë3FGL J1514.8-3623@tÊ # –@2Ù_'F—À9ë>nИ3À;‹<R–¥É?ê©idð@oèך[6@=¸¸ÇÝ?âºT£‹¿ç,.õ¿gè¿ælõùÕ¿í/_[&¹ AGNbcuPMN J1514-3617?æN®ÒŸ¶?ÊJj¤~?Óãb¢ZÀ–?ÊJj¤~?éÌþ£ƒ'?Å­G¤E6l?ÈÌqó…º?Å­G¤E6k?åô[–´Ó€?¸Õ…oÿ?ÔHҖY?¸Õ…oþ?à56ev^?¹u͇?Ò?ߕ"5ýE?¹u͇?Ó3FGL J1516.7+3648@M×­€k`@Lô¯ÀL‹ÊÀ:s[Ÿc6À<
ÅÓ´G›?ã'ã鸯£@Ö;‹qc@שjÄD¿Ø‰Ö«Ñ]3¿â­vû¿åuÒùüI¬¿ïþ;g4A¦AGNbllMG2 J151646+3650?î9~6»ö?·WþHu$Û?¬h"@Ÿ¦?·WþHu$Û?í3ƒÆÍ÷?¸w}£üáï?·îcáɐG?¸w}£üáï?ê !ô>×?¬¥vþà'?Åx-û¢?¬¥vþà&?êlmØa(`?¶I	pƒï?ÆNHž{^"?¶I	pƒï3FGL J1516.9+1926@;՘Ÿž–Y@KëÀ·pDÀ9Öï
wÀ;µ"'±ÈÀ¶:¯³â@ül¦œau@#ìÀ24±¿ænž¯¿1¿êæíZ¿çû÷–5GF¿ÜÛý`':œAGNbllPKS 1514+197?ïûw›	ô!?G~x²²'¨?B!"Ø/zÌ?G~x²²'²?ïÅÀ—†?‡‰zŠ:?}´<øz?‡‰zŠ8?ïLBàä¹Z?Ž)žó@d?–w£ãhÔÍ?Ž)žó@n?ïÿ"T$kí?ØŠ¼ù?êöåÊ?ØŠ½°3FGL J1517.6+6524@YÛa»û@F³'Àa"À9OŽuy)À;L	ÃÎ!¿õ`‡·™ß»@sIcKSæ?üƒ—
&Y?{­5F¢•…¿ã-dÃ2¿Óƒª3ða¿Â~	ZÇ¡ÀAGNbll1H 1515+660?ïýˆeÁh?4õ¼Ü«'µ?3¼Ñ÷$½à?4õ¼Ü«'Ê?ﶱÎ[X?…ò¶½©?'SŒi)üy?…ò¶½©?ï¤ë~L¦"?…8˜'I6?†Å lÖw‡?…8˜'I4?ïÿ¦ Ÿ*7?
Èn¬ñÅË?wØ5r3"?
Èn¬ñÄé3FGL J1517.6-2422@uJÑ"Dž@;"§@KIªÀ7es!_ÌÀ:ÔÖ-žž¼?Õû¶_"$m@eÓ|"P/@å±_³ï±¿ã#oڔœÁ¿á¨ãîžÑ¿à
¯€ƒ"¿æ"YO@tAGNbllAP Librae?ïÑ󆽍?x‹±¢†;ã?w<¡9r ?x‹±¢†;ã?灯Ÿ7"?ÐfPRU?Ðü Á'àù?ÐfPRU?íx¾Ñzw?£ó"8°?´?*	t,H?£ó"8°?èª}M²pf?¼õÎ%?ÍV
É6>i?¼õÎ%3FGL J1518.0-2732@u*­ ‹]@8ùx¿.~™À8šRÙÀ;$C£Ã¿¿À€+q'Æ@"ÂLÁ#Ì@‹Ÿ°ßÜ¿ÞcS÷ÎÙ¿äâ=X¿Î{¿àÃQ,(¹¿â>*þ0rAGNbcuTXS 1515-273?ïÿ½ô,ü4>üåîÚ8+?'ôÀó*ó>üåîÚ;?ïÓ"Áf?~ç'"¬?vp½Ÿ@Lš?~ç'"¬
?ïÓªàÎ.d?y‡þ?@Å?v*˜èÎc?y‡þ?@Â?ïí|A7-?Y2?`®J?bƒá¾ÈÒ¿?Y2?`®S3FGL J1520.3+4209@QG¿@OÂ@L_×ÖìÀ9³—>u‡À;ÝWªå?ì/xB~L.@5¬µ*D@ýXÌ¿àv›"_aÔ¿è¿\"ÞýZ¿çCvý<½¿ìPa¼Þm3AGNfsrqB3 1518+423?ïö›5-OÅ?VT~é96'?Rɕ¥`u.?VT~é96£?îêÛ|jûÚ?¢ÜÁ–Ñ¢?¡RH9PBH?¢ÜÁ–Ñ¡?îȀᤄ?™"¤{¦0A?£wñå·¾?™"¤{¦0@?ëµUPUeó?«ËLã´¥±?Á*ª¾ªh3?«ËLã´¥²3FGL J1520.8-0348@vaä?åÉ@E@Ì?ß À8ñzbœ­JÀ;B…¶Æ?ìù×	Å.P@þC"¨"Ý?ýXà¨Ì½?æ6Ãì±ø¿Ø¼c,9ͿΕE=-­¿à$¡Vk5rAGNbllNVSS J152048-034850?ïx퇺m?f›T½]ˆ?ýâO²€?f›T½]ˆ?î'hò®JÛ?©Ûáä‰=?§ÙpÕRH?©Ûáä‰=?îr'µK'?œ £¡@|^?¨Öçä«FÞ?œ £¡@|`?ëóE¾Æ?­ó¹§±®?Ãü2éìæ?­ó¹§±¯3FGL J1521.1+5543@V‰?ßéà@Id›`C6¶À:{7ýJCÀ<#ǃ·°?á&D"He¹@
È—ý¸'@]+éTm¿ìQßÅC'¿Ö.î"Fe¿å=äð¥¿Ô?Áœ"[AGNbllSDSS J152034.98+554256.9?éò"WâßH?ÍSüáœ?|?È5® t'Ý?ÍSüáœ?|?í÷²'|?¸È&ø5ã¿?°Bo+s ?¸È&ø5ã¿?ìöø,d?®+yg»ëv?¸H?.Ÿ4à?®+yg»ëw?ëÃîjÃl?µ!–ªYš?ÀðFTòN?µ!–ªYš3FGL J1521.8+4340@QæïÝëÙ@KÉN ƒyÀ:$ìH"ÉÀ;×#{/K?×ÜŒ{›@u^>#Ò@Ú÷àvͽ¿æß+‹7ðÌ¿ëš{Òðd¿ç^õ }ùֿڕTV0ŸAGNfsrqB3 1520+437?ïþöS?X?&;Ã{{Û? šÎ\
}f?&;Ã{{ÛI?ï†ý=nwø?™<ý¹h:?Ž@°¤b4?™<ý¹h:?mhڀ?†Ñz­U?‰˜¤¥É`7?†Ñz­U"?}p¸?€â+©GË?‡P`£ù',?€â+©GÊ3FGL J1521.9-5736@t VàL'¿Ûd _þº¨À7d˜$ qÀ:D˜n#Ê@d—.Z[@Xç×Nl@=Ã/@¿Ï•¦'Gã¿áǼ¸é§4¿è}M÷7b ¿í ÞW
ØÜPSRPSRLAT PSR J1522-5734?(×Ðòž3Ï? ·qíÇX?ïþr'ðÖ? ·qíÇX?-X)9UÐ?F "vµ?ïþ*}lj­?F "v´?s×çª1±ë?^ÛnÕ]V?ïØP0«œ›?^ÛnÕ]d?Wì"
oÔ?MÐ%—M?ïô	µùH?MÐ%—N3FGL J1522.1+3144@IÓßæ…@L'ßý`éÀ6FchÀ:£ÓöeM?û¨w³?Ýæ@…éµí¸@~ÓnQ—L¿âN¬Œv¬–¿åʍ¿	¯p¿æ]J "'¿èÏÅÇíAGNfsrqB2 1520+31?ïà1ø;?nv˜ÜnÙL?oÎÄñém?nv˜ÜnÙN?ïͤP	"
?†xÎ.:?y-×û5ûb?†xÎ.;?îË€'C¼?œèËíâã?£OGý‹Ä,?œèËíââ?ïütàVÝ?BõOšÖο?<XýO¡·?BõOšÖΰ3FGL J1522.6-2730@u9\_|gZ@8f6îÍ©À8$l"}ÐæÀ;žîm0…?ò³üY,l@Öâ'ܼ@"à)ËÖ¿Ùkë[-M@¿ã^¢;˜vH¿àTË«±ì¿æ´œ.ÊBÚAGNbllPKS 1519-273?ïûò•²d?@ïÈ!¼F?@5«½6k ?@ïÈ!¼*?ïÍý^ºo#?€+O,4ž&?yP¢Èo%?€+O,4ž'?îÿS¤XP?—."ßâ? 
ź;?—."ßà?ïmw9N
?ƒ¾b'"Å?'QÖ>¾?ƒ¾b'"Å3FGL J1525.2-5905@t8–ž=¿þm)Tc¯À8äç
À²ãÀ:QÎ2þZ?Õ®ËÄu@
½U5'@JÛ`cm
¿æHP¯×ï¿æ©³ÍÍRÚ¿ç
'¿ç-BÀÜ1AGNbcuPMN J1524-5903?טö?Gq?Óp¨¤¥ÜS?ä3"à\Gt?Óp¨¤¥ÜS?ê_$¨Ñ?ʹþ°̧?ƃoÝ\¹Š?ʹþ°̧?âÂ	è?¼–ZÃ6`?ÛÞ{ïíÀ/?¼–ZÃ6`?î
8Z?¥q?µ+¦k?¯/<z^Å?¥q?µ+¦k3FGL J1531.0+5737@VæPß´0@HS?Ýe¡À:y¿ß~€À<¥šXÜ:?âÛ$»#ù@q|ï>çœ@%±ÀVò«¿çíÐ
¿áœF7¥f_¿åRkuwƒù¿µÀ½mÍAGNbll87GB 152947.5+574636?îJÉbor£?µŒgŽ/W?«SiÙÕÇ?µŒgŽ/W?ïYO­@L/?¤1g8VA?"Ö
WözW?¤1g8VA?íÃ{ÑGw?§'fÎÁ´v?±ä'uÄU?§'fÎÁ´x?ﶕ«•?—èÈÌB(3?¼©-J^?—èÈÌB(33FGL J1531.8+4704@SýÀ?`@Jr¢ŸÒ˜¿À: NRsj[À<ò¢Ik"?¡øsìý=@
ð*IÏ,@†Aßsm‹¿ëÜõB¦‡ƒ¿Üò4@à¿æI§­Û¿Ø
«(t‹AGNbll1RXS J153148.8+465912?ígÐRð¼ï?Â3f™ä?´Á}hzŠ?Â3f™ä?ï>·Ä Lï?£JêyW/?˜)köb.?£JêyW/?íue_Íþ?±zth¶lw?·|TՐ?±zth¶lw?ïMî°ÐvI?Ž üFŠ×š?–B)åñ74?Ž üFŠ×š3FGL J1532.0+3018@Gì:?–îÄ@KhZ&–mÀ:!=ÍÀè"À;´:ƕ?Õe™W)‡Ž@[¦nê?ü>AFœG?ï÷aÐu‡¿Üh‡Š…¿ÑY¤£°@G¿× ‹ŸÊ¤îAGNbllRX J1531.9+3016?ïßjïk?xÒÃMP®É?pJöôJ¿?xÒÃMP®É?ïrõ¢ä˜g?¤õŒßpÞ?'¡K£lòù?¤õŒßpÝ?ï@½Ð=?–_­bV¤?ž—ýhEøD?–_­bV ?ïc']>@¦?Œ}"¡"Ãö?"´X7ë,?Œ}"¡"Ãö3FGL J1532.7-1319@vHÿ¸²d@@Ü
`:Ó;À7Ý[+J1À:êè'œ&<?èݯr–Aî@@‹Emó@À…Ü.?¿×!R¦ý¦¿á"­Þ8ô­¿ãÄUã4¿ßó¶ËهÆAGNbcuTXS 1530-131?ïý]þŸ?7þ'Îû?3•
þ6?7þ'΀?ïØâNÁÁF?|_™t€.?sŽØŸ]Û?|_™t€.?ïUgdš,?'&¬^º@^?•NSlº–?'&¬^º@^?ïÿþÔÐÞG>¬òÆrËM>¢²ò‰iû>¬òÆrË6ä3FGL J1533.2+1852@=)@ªÀ3@Jÿ—$tÀ:0;eÀ;¹ãÕ'b¿ãùB¦Ì;@
ŏb^?þOà2ZE¿é†lêJ¿åÞŸ¦Eq?½‰Jl	éc¿Ûù˜áýzXAGNbllRX J1533.1+1854?ïþÆsøªÊ?!Î8E²p?#˜ÀuSa?!Î8E²»?ï¯2×
û¦?½›´úC?"3J=A?½›´úB?ï¹»'5b?~AAñƒ?¿'²§¢?~AAñ~?ïúT®¼n?K+ã~i÷ð?F­EùFæ?K+ã~i÷ã3FGL J1533.5+3416@K_{Ÿ³@KU@ÿ¤nÀ:lÃÕ­FÀ;ÕòJ4×x¿Òɐjc@¸©Ý3¢D?ý«:ÞÎ,¿ãSÛýÊÏ$¿ç$8vi¿°T÷†½R¿ànG˓RAGNbllRX J1533.3+3416?ïý‹™k?9z'>\'?3§K7¦{?9z'>\'#?ïŽó‡}Mã?'ô("7ý?ŒC ¬‡ ?'ô("7ü?ïº`«dã?'Nk¤å?gÜ&Ç>?'Nk¤å?ïÛÃKÍÐ ?q³RؤHº?rZðˆ?q³RؤHº3FGL J1534.4+5323@U`7ßÕ¾
@IE`\a*À:׺nü7À<!x#'L¿Ý•VpqyŒ@uuœ9\?ÿZÞ°t|¿í9"ZÌf¿­š"i´¿ÐIÀ	è-ž¿ãŽ…ÎØâýAGNbll1ES 1533+535?ïÆqGá$?"ϯo¯8?|ÇqÜmË?"ϯo¯8?ï<«UÎü‡?¡K…Ð!N?˜j•F o+?¡K…Ð!N?îs~L§Ÿ'?§}W$Jˆ¨?¨È5†Ð?§}W$Jˆª?ïÁSžl›?xÕó£Ì?V0¹I²ô?xÕó£Ê3FGL J1534.5+0128@´‡ßÝË£@E¢¿ÖDEÀ9r´€ÈÀ;9oV•¿÷RH¿·e‡@ä8¤6V@:Ä@]׿çõ*åd{Þ¿ê%…sÌοã2¶¨ö¿ïÿÂáo#ØAGNfsrqPKS 1532+01?ïÿÔµ>ßÈ>úÑ3TÀ>õ¥`
>úÑ3TÞ?ï¼²z9`R?ŒÑ¢ü
j?€Óaq§ë¼?ŒÑ¢ü
k?ï°²›\j[?­oêÿyv?ƒÓY(åia?­oêÿyq?ïÿ  Ŋ?U"ÈØ2£?þwΝ^?U"ÈØ2j3FGL J1535.0+3721@N: þ¡@K.ßç[ÄÀ:kc%iFÀ;èa'ÑÖø¿×IñàO@UáŒR3@é¾ RÔ?¦:A^2ÿö¿ä0+Y¨›s¿è¨ærT+?°+n"ï¼AGNbllRGB J1534+372?ïS¶qÉëù? ¨B¤. ?•‰1Æ€æ? ¨B¤.?ï""èúª?ùÇîi?‹7OÁUt?ùÇîi?ëû^W8%â?´ #–î•ã?À†£hr?´ #–î•ä?ïԓсTã?sÃ~\>£þ?u¶?Uä?sÃ~\>¤3FGL J1535.7+3920@O«"?½…1@Jó®ñðÀ:§ouÙ ñÀ<bfýe?Ý©¥wÀ£@@d•Xí,@Ë.@/E?ïþ¼I$"½¿Ý³"ê÷Á¿ç>Ԁd-@¿ßÓÜW>ÅAGNbllRX J1535.4+3922?ïVøÏÂËá?švb€døU?• 榃´?švb€døU?îꊍT?©`tá¶o3?¡W_ßÇ*Ð?©`tá¶o3?ì['¶0J,?²"xxc?½#jN}® ?²"xxc?íƒ7mê®?¨Ž'ËÌC?³æDªB?¨Ž'ËÌD3FGL J1536.3-4949@tƒ!_Ìr@ Þý';À7)&p­À:"&êþ@&»¶Où@y6R!Šê?ù×2
ï+ò¿Ù+¹öËпÜh‡#±q8¿àKª7m÷Í¿é=ORòPSRpsrPSR J1536-4948?©c`£¢?©9w£¦c8?îniÉÿ…Å?©9w£¦c8?d#]ꢪ?u¼IŸ	tÏ?ïëÜ¢]V?u¼IŸ	tÏ?Ð9P'o?µì>»Ñt™?çãrW·7É?µì>»Ñt™?mû=Š$L
?`'~ÐH
?ïâÂuÛ³?`'~ÐH	3FGL J1536.6+8331@]z÷@?åğס<À:~†TBwÀ;ýF†Í;¿ì°ç¶Tˆ@ìF±c@ÙH@`˜F¿âD÷\݇¿çð›nª¿æboð9Á¿àâf¾O%AGNbcuNVSS J153556+832614?ïö'¿R­?bÖÓ ¹æ?Rú€ßZ¦?bÖÓ ¹ç?ï'+ý'PÚ?›bÆ"Nò?‹u¶+ÉT?›bÆ"Nó?îÿ"Þ¢0?"%"a¯˜i? ¿ÒÝ?"%"a¯˜g?ïҕçQ—g?t@.!Æ/?vµW4LÊ?t@.!Æ.3FGL J1537.8-8000@s_<`ŸÀ3}_²?À9CÖNUÎiÀ;~æ"ôï+?Ö!ª°ÔYð@KÚsÿV@}Ç/$Ü¿á¹SK~ó¿ãgâ(Ý"¿àRÁՑ±2¿çœì='AGNbcuPMN J1537-7958?ïóߘã?b—=\"ü1?X@ÏéÌ9‹?b—=\"ü3?~iQ?'?Ð/vë?‡\x e«ø?'?Ð/vì?ï¢	Ðyó?†Háç»0é?‡}‹á¼'?†Háç»0é?ïn{p?üÙ?€¶êè¹á?'0'ød¼?€¶êè¹ä3FGL J1539.5+2746@Eôv?ø="@Jqÿ΁ÙÀ9O~Rì6À;šÌÜ­?é(·²ù@Ésô–$@©:ÿZh¬¿Ílï)÷}Ù¿à¡_ðÚÕ¿à›Ôÿ˜ž¿æmá|S°AGNfsrqMG2 J153938+2744?ïüÌ'Ã6ý?=UÅK8{ ?9žÁæH
w?=UÅK8{®?ï·}6ÀÅ?Ž|'B˜^m?' ²Oο£?Ž|'B˜^o?ïZþ¤Ó×`?ŽLqj_f¹?" +e…þ?ŽLqj_f·?ïø172Ãt?Fã 
'œø?O;#4ò0ó?Fã 
'3FGL J1539.8-1128@v2ï€Uûµ@@çk b
·À9ò¬U^fÀ;s×gZ'¿µc9ìLÿ>@
°R°Ñïv@­Ó %¤Õ¿êȆ)þ¿äj©…䠿ݨ"õèF¿äé£Rˆ–›AGNbcuPMN J1539-1128?ï÷Ûódæ?Z+2S‰'K?PH6xµ€?Z+2S‰'J?ï,••ÌÝ
?£Á»6,å?šmMFd^Ñ?£Á»6,å?r@É?†¢ÙՄvÌ?ŠÒ£¯Î-?†¢ÙՄvÍ?îËÙCa.-?œÿS(šáf?£BkÉí<?œÿS(šáf3FGL J1540.1+8155@]—¿¤Æ@@{¢ò(§À9‹QÿÅHÀ;}êXÎÎ?êú"9!@T6
-?ù¢ºÀèG?ïøœÀ¯K÷?£B†jñC,¿ÛèQHÙ¿°wËNٓAGNbll1ES 1544+820?ïÜ `öÆ?rŠ 12ãú?q¯ýO"ˆ?rŠ 12ãû?ï®\•Û'?‰ ÑàïÅ0?"hډ;ÛÕ?‰ ÑàïÅ0?îm†–a?™¡€Kq¾?©&÷–öš?™¡€KqÀ?'ÄÌ? ÕÙ³© ?¦ônVã³F? ÕÙ³©¡3FGL J1540.8+1449@8`Ÿþ7©@Hhâ:¸cÀ:œU5¼À;xÔu§L¿°Çñm<°@DYgzb@ÂgŸÌc›¿áè+ðɬ1¿çPÐò@T¿éØi€¶}¿ª­eÌô¡AGNbll4C +14.60?ïáBƒ3=™?€ÅX§Òé3?n½|ÌÂg?€ÅX§Òé2?ï£RS
‹l?‹?6âw?‡+k=]%?‹?6âw?î'Åü'çc? <ô'Õ>?¦Ó 6щÑ? <ô'Õ>?ïÌLð·Ç@?u‹
lõ	5?yه¤`4?u‹
lõ	33FGL J1541.8+1105@3Š"€,á
@Gw±ÿÁìŸÀ9ÊÂñ·üÀ;§À)P[b¿È`®Å›@P‹RY@Þ1àwÏo¿ç>O"ùÝã¿ç
dHI…¿êÛí›=L€¿ïþÉ|w±AGNfsrqMG1 J154207+1110?ïøíü"d?L'«?LH¡®nH?L'«?îB6ï‹
?²Yƒcö?«ÜŸOp?²Yƒc÷?ï^Ô܁©?‹œ	Þç*¹?"%}äoÊÇ?‹œ	Þç*µ?îcŒžÅa?žåÒO±¤ñ?©Ïw6©í?žåÒO±¤ñ3FGL J1542.9+6129@WØØÀ  @F²`œ˜RÀ7Óû-2h2À:ì³Z§?óòÈê•	½@~b«0E?ýKê"_¿Üؼ'@¿@¿ßû)ñëë¿ßJ:-DÔ¿â½'{Æ}†AGNbllGB6 J1542+6129?ïþYjpM£?-¨Ù¨q- ?*iXû%»"?-¨Ù¨q-?ï¼kÚW®?k
t@£ä?€û¥	jƒ?k
t@£â?ï)ïƒ&ß?"XÂ%ü…?šÂ›?"?"XÂ%ü"?ïï²iÙèÅ?Y~—Ã)?`M–&;'?Y~—Ã#3FGL J1542.9-5141@t~œ…×E@Hm`€žKÀ8Œ7ùk'IÀ:­AÞËÓ?êaV8¾.ò@
h•»=®6@èMß[ð—¿átŠô¿èÝ(œx¾z¿äˆJYj{¿íÒç‹BûPSRPSRPSR J1543-5149?Å#'{ðÀ?Ãâ1íŽæD?ê¹w6!Ð?Ãâ1íŽæD?Êgþ1{à¿?Íå-»‹H?éfs¡Ñ?Íå-»‹H?Þx©&Áqi?¸€j(%Y1?àëlŸGK?¸€j(%Y1?˗°é~8¢?²FN6[?éÅ qØ?²FN6[3FGL J1543.5+0451@(|ȵ1¦@E²NŸ CØÀ:,ÅÜÃkÀ; 	Å{Ÿ´¿õºD²6žx@
¸TûÛ?ÿÁàþ¿ëL "ö¿Û±WšŠt'¿âTÃRß̿ĸÞAGNbcuCGCG 050-083?ïü';â?=(
ƒrZ×?;î$ðø!?=(
ƒrZÝ?ïÁ'}ÐW=?ŒãÕ®2¶?>ÁÔaª?ŒãÕ®2¶?便Ý<©¥?–@Íè?†–ˆ°Õ—?–@Íç?ïþúym2é?#byQE)Š? Xi,Ñq?#byQE)•3FGL J1544.0+4938@S̸`.>@IŒÕ£5À:Zäd™ÍÀ<åB¿Ã}}!éµ@'‰¹QÅÅ@j¨_°ٿ׻ϣZ§Z¿àe-Qzy¡¿ëòÀb—`¿Ã‡­,@ŠPSRPSRPSR J1544+4937?ïô§™×íÖ?YñÈ2!{?V°ÌP$OÕ?YñÈ2!w?ïï™u׊¡?t´:§APÌ?`fŠ(u^{?t´:§APË?ï^°€.×?"r÷I·ý?Ÿ)ïú%4?"r÷I·ý?ï߇{Hk¸?rÓ¢"Áh?p<B[Ê#é?rÓ¢"Áh3FGL J1546.0+0818@0ÄßVø4@FWM@$³>À9°åÜhKCÀ;`üÀ°^Ø?äfIyà[@šÁq¹?û
i€L@ ?ïî
ñº[Ë?çJü©š~Ø¿×XŠå:›¡¿Ö<]ÍÕOAAGNbll1RXS J154604.6+081912?ïù·>6?L[â;‡7j?I#ï»&õ?L[â;‡7f?ïŠKÜëTá?"ï5#¡í¿?mÅ*Ǥ?"ï5#¡í¿?ïE¡ù?'9ð)èÚ?—\«ÀÞ9?'9ð)èÚ?ï#†21 Ú?–ŒOžï§,?›9¹Ëä¬?–ŒOžï§-3FGL J1546.6+1812@=í2ÿ0Í'@Hg¥€W©4À:Gç.wâÀ;»Ä4wÖÑ¿Õ¼ùßÄ:@
Yžk˜y@gnåhz¿ãÉÿ&
}¿çf¤¢"È'¿ÐoXÞša¿Þ~K¸˜ÀßAGNbllMG1 J154628+1817?ïþNÇQip?1(${¿›?+Šéhñ.?1(${¿Þ?ï‡˓Ğ?"Ò¬ZÀ?Ž>MØ)?"Ò¬ZÀ?ï[ñ/¶º?ñÑG(`Þ?"Ú‰(ã?ñÑG(`Ý?ïã7ÿ©«2?d²ôÃMäã?lÈVTÍ?d²ôÃMää3FGL J1547.1-2801@u|€àe0@4•2Ÿ|àÀ:MÎ_ªÀ;ƒcÎÜq…?ë'éýÎç@
üF£ÓYY?ûRÄá
x¿ïÍ3Ó¨Dh?ïø5£®h¿á&¸ê¨æû¿ÝG:SZgwAGNbcu1RXS J154711.8-280222?ïÓCY@Ø|?t¥y¼dÓþ?v^S_"Â,?t¥y¼dÔ?îª{D½¸?°fO%	?¥^8K´$?°fO%	?îiBbÿOž?›¬9ü^wŠ?©kÙÐ?›¬9ü^wŒ?èò×È%?¿J"ŒŒÅ¼?ÏÜ4 ß‡k?¿J"ŒŒÅ¼3FGL J1548.8-2250@u½¥¶™…@8*% Jù#À9|©žÊ[À;?fg=%û¿Ùà Fåu@'#C¦óÊ@b#¿ø¨ô¿ÙûºÁ1Ž¿äcíÖÝ?¿â¾ŽIj"X¿Õôg25©§AGNbllPMN J1548-2251?ïïãwÙôA?]r;Lž?`ˆ&½ù?]r;L"?ïÏE3¥?~zÍZ·‡?x]{ðæ-¡?~zÍZ·‰?îìrãy"?—qëÁz~?¡8ÑÎ(fÎ?—qëÁz~?ïÄC/³ª?wÏ£NÖrz?}ðÞh&+O?wÏ£NÖrx3FGL J1549.0+6309@X9Àgn@EùJ?¿2°À:iêÝYÀ<‹?cÃÀ8‡Q˜y@›@"Yò@Î8£NN¿æ@Ç/ÿÌÿ¿ìpژ½P®¿ÔùT~¡4‡¿èƒdç"AGNbcuSDSS J154958.45+631021.2?ïû¨ºó9Ê?KftĴב?A]3Õm?KftĴׅ?ï–Õè<4?¥ØY@v¶?ŠJ…ðòÿò?¥ØY@vµ?ï¤vW&?–W•WO?‹q5<£?–W•WP?ïþ²ß€éL?5Uä'?$Òñk+1?5Uäs3FGL J1549.1-5347c@tuè_ÐJ0?Û¨h r2ÅÀ7p@Õ³%\À9ý"'¤?ò1˜Ä1²@ŽG…z©@xǟfb5¿ä̬¶¬Ï׿èD®?îØe¿æïçCp˜¿ïïå|OTHERsppa?•¡__{‹?£vÃu2Ö?ïRô#?£vÃu2Ö?}"OñÖwF?Xߎ
@?ïÄ×`S?Xߎ
@?Ç!\‡ƒ'Û?µ½ôð^Ç`?ê7¨Þ‰?µ½ôð^Ç`?¸¥è nä?ªÛ1s¡:2?ìëOÂëò#?ªÛ1s¡:23FGL J1549.4+0237@%¸çÖyõ@DtÈßØBLÀ8j™ç2«À;UýgŸKŠ?ÛÑ^$@ÑIOL@´é •vÊ¿å;ßÊÞ鎿æGkX,€«¿åÉ_›'8:¿ë:ui0AGNfsrqPKS 1546+027?ïú˜ê1T·?J/Á"özz?EœW:­!±?J/Á"öz^?ﵸŒë–?‹ç€A"c?''ÜÅz'?‹ç€A"c?ï_ý˜±øž?Â
o‹?ü?"LéÀìi?Â
o‹@?ïê¾ €Ë?^Ì
2:Ò?eAß4q(?^Ì
2:Ò3FGL J1549.5+1709@<ҏÃæ@Gç
€CRÀ:–ŠQýù–À;ג'µP¯¿âjڋə´@f÷ºâ±?þ¨›ÿÊ{¿ë;iå™CÖ¿ÙS'Bï$!¿àü¦Mÿ^½¿È´q'¥šÀAGNbcuMG1 J154930+1708?ïü»üþèô?DI3ªúu?: ¸b4?DI3ªú‹?磊âPóŸ?þW½!Ô?†žkÃ?þW½!Ô?f×O?S9±a?ŽÞ&J ,,?S9±d?ïýÅiN?6'=	Wµ¶?7Y×ĵ"J?6'=	Wµá3FGL J1549.7-0658?ó˜OÌû@A¾ß¤?æÀ9;´L£FÂÀ;DD<oò׿î求÷õ"@ëUN.?þÇÑ`w‰¿ËðzÑØO¿àkI]ǟ¿â¨ëy5K¿ÌØ¢cÒ§AGNbcuNVSS J154952-065907?ïèÞ-´Sm?gvà»þ~§?g!ÒK¬'€?gvà»þ~¦?ïѽ±9ò?'ŸîFb 3?w|!'cm?'ŸîFb 4?îÿè'9W?'ü™óV‰? wÜj†æ?'ü™óV‰'?ïúS>gj?J¦_ÿ?F±ÃbZ?J¦_ó3FGL J1550.3+7409@[8_á'p@B×@&`½À:oË
Tí˜À<¶ŸcÝö?á‹b¡àºë@¬P¥^ô­@›@bƟ¿æz\q½T¿î1=#:Üd?·ß¿¥"F¿ãìüÝAGNbcu87GB 155014.9+741816?ïý½¡5·?Q|©C1Ïî?2öW2?Ð?Q|©C1Ïó?ï°<ï±`P? D(ãñD?ƒðħì? D(ãñF?ïEHZ9?ž#^E3Í?—Vð"¸æ?ž#^E3Í?ïÙ	µÓ<ý?vú´¡?s{%aq?vú´¡3FGL J1550.5+0526@,gÀ_A@EÜà@GÀ8à€If{_À;n"aKts?ílÂ|*¸@&wºL@¯ñ⢿Õ.J ã¿æáNö‡¿â$à"¿ïþÄö¶ørAGNfsrq4C +05.64?æW|+œ< ?ÉóY^ê?ÓQ¨Ç‡À?ÉóY^ê?ÃEØhu@?ÆkU¾aÃ?ë.‰åüâ°?ÆkU¾aÂ?àþ@`è?ºËބöÛy?ÞÝ×>1?ºËބöÛy?Ñ_ó0?·?±Y#,'?çPg¸`%?±Y#,'3FGL J1551.1-5610@tae¿­)™¿ù­1@ê«ÛÀ9²`9ü{À:" z^jï?í·ºbM8S@Ë îؐ?ü ¢qON?ïwÌT×È©¿X3¬Äˆtr?‰7º£ÌŸ¿Öþ«OTHERspp?í‰>؈.î?´á–‹+?³¶	;¾ˆ–?´á–‹+?èè´~ÕÎ?ÑÁQI֎?Ì_•.¨Ç?ÑÁQI֎?ëÈÍVΏ?ª%ݯ=g?ÀÜʤǵÃ?ª%ݯ=gž?íc¿ñ>?°í½Æ1?³âv?°í½Æ13FGL J1552.1+0852@2q_¾¬y@EÓ7GMœÀ9õäžz©êÀ;¯%v²?¦šXmjÁ´@ÿ-ªˆ)Z@®{`sˆ8?'`ÏÅòàT¿ßŠµâ5ÐÙ¿éñ¡À¯ˆ¿àé¡r¹–AGNbllTXS 1549+089?íÙ18ˆ÷¹?´Rü
ïòï?±6v;¸B+?´Rü
ïòï?ï.ømäý? §ÀœìÆ'?š òCÀr? §ÀœìÆ'?ëø@ÏK<Ø?³£($Û¹p?ÀüÂÓ¡?³£($Û¹p?[Ÿ÷?™UohQåx?¤WúNæ‰?™UohQåy3FGL J1552.9-5610@td•`"¥¿ü#pÀ\|À7'¨|‹kÙÀ:LÔ¯]Ÿ?Ö.]pžx§@}Ñ2¸$@@YŠ¿Ýw¨Ãƒ"	¿ãÎ6YXa¿âo¥ßøù|¿àŠÝâɹOTHERspp@?æé¬a×?Ï+‡>-1?ÓÆ-Ô§<R?Ï+‡>-0?ĽèBt'ß?ʗŸÀ`.?êЅïbÛI?ʗŸÀ`.?ç\Ñ)ˇu?µP@ñA+A?ÑF]¬hñ?µP@ñA+@?Þs^~W+!?Å»^´,<?àÆPÀÔjp?Å»^´,<3FGL J1553.3-2421@u¸ÚŸ¾vÉ@6Z(Àª'À9YêPkR^À;WªÒ§a?éwØ?á[>@½¸Ûÿ@<_":4¿Ì[>¿çÓSà¸ù¿ào ½Ëä+¿î,º~t,ÖAGNfsrqPKS 1550-242?íßÀLé¸è?°˜£=Î?±ý˜²8Á?°˜£=Í?íšù¤cVæ?¯È"š=‡©?³(2ÜåHÈ?¯È"š=‡©?çSù\Fü3?´9QU.°p?ÑX
Gr™?´9QU.°p?èUCÆïÊn?°'dGš?Ϊðä@ÖG?°'dGš3FGL J1553.5-3118@uieà.©a@15·?œÎÀ9…àãÛKÀ;Oûx±Â…?ø(0…ÙÉ5@>4r"‡>?"3/ë¹Á?éÇW±(Ó?ïû¡ék¶T¿ÓSM©oê8¿×æõU_¶}AGNbll1RXS J155333.4-311841?鞅øKªH?Äø]}Òyû?ɅèÑVã?Äø]}Òyû?ËÁ–«1^?ÔjòjZV%?霚U3©?ÔjòjZV%?ç/ØW%Õå?¶8+×¹X?Ñ OQ´T7?¶8+×¹Y?ώ%×Dx0?Âw،cäö?èvŠ.áô?Âw،cäö3FGL J1553.5+1256@7ɁOP @Fœ  0÷ðÀ8;‰‹.œËÀ;8±0?õÄ>£©½Ô@÷A\k»»@ÅÂnoI¿â]ÜT)¿ä")y1U¿ç+µª¾§h¿éÿì²£ßKAGNfsrqPKS 1551+130?ïëOö/?dxíÔRŽí?dâ°	Ðqj?dxíÔRŽì?ï³	¸wzF?Âø©Ì?ƒ='â!nO?Âø©Ì?ì±ó5NØÁ?§ùGÛ;?ºpfU‰9÷?§ùGÛ;Ÿ?ïìàc}˜ ?^œ=g?cœ'g^˜?^œ=j3FGL J1554.4+2010@@ÐÖ 2¥o@Gß<ã.À:E‰bÙÀ;Êô¯iåw¿ñSÀßIý@–Ehƒ@¢à?Ee¿æa‰iÃ	¢¿âԗ.Z[k¿×&;ìϿ簛µ
ú{AGNbll1ES 1552+203?ïì›v>ãN?k´&ãíE³?cd‰Á²?k´&ãíE¶?îéĚgŒ?­±ùŠ¤öÒ?¡nöY‡A?­±ùŠ¤öÓ?îåuºrc?›v¡N×ü›?¡¨¯tXÙÓ?›v¡N×ü›?ïÙ'ÇþÐ?u,g"?sl9—ë?u,gƒ3FGL J1555.7+1111@5ë€uf@EúÕߛªÀ6‡ÜŽá¯³À9Øoàb«Ç?ëXlQ?–@DGw7ïÛ?øO÷øµ¿Ñ$¹»Öô¿ÚbR'¿Ñ§—U"þ¿ÑAЉ3´§AGNBLLPG 1553+113?ïP`Õ$Ùò? ÆT\ìâ?•óå[dÁÏ? ÆT\ìâ?«òM?™:?½A ?y¬Ã?™:?½A ?ì{ˆ"®E?­Ž-Úø?¼#»_jä?­Ž-Úù?ï#ãUò¬?žzœÃÚî?›ƒ•G‰ª|?žzœÃÚî3FGL J1557.4-7040@sÓIàâiÀ*QGàiaÃÀ9²ªÿ«1À;¦™_·öÀ	)^€"ä#@çÊ´èª@h(ÿӊV¿åx­Áä}¿â¿"nÑ3¿âÐ*æô¿æg¨MðŒAGNbcuPKS 1552-705?ïäU¨Óùƒ?sÜݧºï?kªW,~Ž?sÜݧºï?ïÖÜÝ'‹ò?†^pô~q?t''l:ñ?†^pô~p?îÞ1‹°ø?˜Šª®_ñ?¢çDþs?˜Šª®_ó?ïÿìG"ä>öœÅFóÙ³>ãú¸Ý¤9>öœÅFóÚ×3FGL J1558.9-6432@tøŸƒ¾fÀ!GŸÕó½À8ÉÄ<ÛR¢À;@cÞÌ©'À¿^\¶@fƒÂ—¿¥@0K`{•Î¿æ륙=dv¿Ö†§qüû¿á}PPB¿ÕÚiýc‡SAGNbllPMN J1558-6432?ï÷Jh›¼?c{ఐf?QËk.ȊŒ?c{ఐd?}HÖ?œ¾O'AÐv?‹ ¿-ÊÃ?œ¾O'AÐv?ï0¸yÔ\u?"$3ŠÇ•R?™èðÅtqf?"$3ŠÇ•R?ïÿçü<Hr>ú'­™i>è÷æF>ú'­™s3FGL J1558.9+5625@UäÉ$.@FàxÀ>-À9DËüÃ4žÀ;´Sø¥˜«¿ñmš}[F@éÊ@®êÖù¿çè(Z½ë¿Þ–÷Üá¿á·_öW,¿æŠt¼P¹èAGNbllTXS 1557+565?ïþñ¯ƒË–?!ü¢±¯? åÃF‰¡?!ü¢±Ö?ï¬Õг?'t9±³+?"ùJº‹Ó.?'t9±³,?ï¥bÈV›?…‹é‡ýK?†§MÿªY%?…‹é‡ýK?ïýØŸ'€?1Æ" ù1?1<Ãôò?1Æ" ùõ3FGL J1559.7+8512@]·Êÿm3	@>TDŸlArÀ9ŒO"}ŠÀ;䰔‡áá¿ða5Tu£@{=gµj@ϊ¿Œƒ¿æØß/®vÿ¿åõ³ö3šÚ¿ß´2¿o¶¿é~ªùF&AGNbcuWN B1609.6+8517?ïüHWðnÞ?Acfú/¸Ô?=½@|‰
R?Acfú/¸÷?ïžTxw?ˆU`ÈUG?} ÕöÃħ?ˆU`ÈUF?ïH¶Ž%¦Þ?"
'|±?–é.;K$?"
'|³?ï÷¸¦7@`?P^¢Tåo?PŽ³'=à?P^¢Tåz3FGL J1559.8-2525@u¾q'l@4'	€²BÀ:lÚÌiÐ~À;ž
ø†¿ã
U€1‹
@€wö[¼i?ÿ-€kË*¿éäåŸxù¿å^â8³•¿ãK±së?­-ZoüÖïAGNbcuNVSS J160005-252439?ïþñ•u?/"ºÔ9®%?.`?/"ºÔ9®5?ïÖ3RÖ/ˆ?~ì[ÓBML?tæV"è<?~ì[ÓBMN?ï²~}^?~ñ½¿cà?ƒ`~ ¨}7?~ñ½¿cà?ïïKhÔ#Œ?` Ú$̌R?`´—+Üu/?` Ú$̌W3FGL J1559.9+2319@CTÇÀ'á@G¸b`GhtÀ9玦 ™À;›Î­wœð¿â"'p³v@µ
eÄ*@ÍÏڀÀ?íÂÀÜÿtë¿á-v"q¿äPcxSŒ¿Õðï
(;ÍAGNbll87GB 155744.0+232525?ïöCeæ?`–p®?Sþýy41¤?`–p®?ï¢(h÷6¸?—¥ä;BM?‡uåÂ2R?—¥ä;BL?îódt;éE?šù‡¶ø? É¸¼Ak»?šù‡¶÷?ïôq~ßNî?T'‰C"]?WAb$é?T'‰C"^3FGL J1600.3-5810@t\3¿µÀu'1>À9ìæ˜Oí~À;KRü&V¬?áE'ÏiÕ@	d^¤P,@Ô?\â.¿âÌ Ë¸¶Ñ¿"îj+lë;¿æ}†Ev¿àpLžÀ—AGNbcuMRC 1556-580?í'ñ×Mq?¶KÇíf?·+èqE"{?¶KÇíf?Ú&Nc$~á?×i¥ü"š?âìØÎmÀ?×i¥ü"š?ì‰+Â2?«
J`ÛÚd?»¶¡îo;?«
J`ÛÚd?ÖQÂEUÓ¶?¾ÛÍí?"?ä×ÝU%?¾ÛÍí?"3FGL J1600.8-3053@uzÿ°Nè@0uS€°"ˆÀ9Цã.8À;É,.\4?÷>¸ŸÄ+@PRþª•?òšª8"[J?ïþ+«™:=¿Î²¢¹ÑB¿ÞTn#°¿ìbÇÒßWáPSRPSRPSR J1600-3053?'™ÛÙ#?–•Ár<xš?ïk7!6ç?–•Ár<xš?§úªÎ546?º*Žü?î€US¬¾?º*Žü?¶eáÿzp?§Uîp+5Š?í3CÀ±î?§Uîp+5Š?»!ænd?¦W ¤ºßâ?ì›ÝÜc24?¦W ¤ºßâ3FGL J1603.7+1106@7ôàM/@EfÀ(yœÀ9ÑøQÆÀ;{Þ-G`è¿©­‰ô1«ú@,f…›
@˜¿aÕ2¿Ïû/i¿æÊ-ªL0¿ãÕÙE"–O¿âïHïíAGNbllMG1 J160340+1106?ïüàDN«¢?E‰Ú¹W8[?8ý݊¢êÝ?E‰Ú¹W8U?蓮"z?o³òr{¿?†xٞø¡i?o³òr{À?ïjQ¯ú†?êQ‡/=?'µÞ*¯!?êQ‡/B?ïÚ€›'?h3sˆ–Í?rð¿²6ÿG?h3sˆ–Ñ3FGL J1603.9-4903@t™€o&)@Œn¿{UŒÀ6üUFƒrÀ:Vól|*?ÖØÛ~@w¿@ˆY«B@«ÿøž7¿ã\̀—¿ä©a÷}
Ô¿àš¹yÞ¾<¿Û+I¡AGNbllPMN J1603-4904?ïåÊè/É?x‡›jÏe³?jå5Ð7Ù?x‡›jÏeµ?ï›;ÁJ?ž©Dz¡f*?‰<q­{&?ž©Dz¡f+?í}¸ˆ
Ž?§üÀÌó(»?´;ƒ¿"ž?§üÀÌó(¼?ï÷Ä,…ë?Nh™m«?'?Pw§ôô+P?Nh™m«?¼3FGL J1604.4-4442@tòߋr@|€.8£À7µ"k4+À:ÃÝo²?ƒ?çðû"'\@7£9€A@Ÿ­@j~N¿ãª]ÒÝÍ¿çå)MèQt¿ã–È6¿êÔí¢QÆiAGNbcuPMN J1604-4441?ïÒ*w·k?|4uA3ñØ?vêÄ$J§?|4uA3ñØ?ï¹É†u%Ž?'hsZð"´?žb¶œ¿?'hsZð"³?ìŽsMO??¨Ú›/±¹?»Œe•†?¨Ú›/±¸?ïÜôöˆÌV?gÆIhlÑÔ?q…"»™Õ†?gÆIhlÑÕ3FGL J1604.6+5714@V(Àª'@F]K 'ßÀ8¦'w"ŒÀ;'ìÝ
?õ"AöðaÒ@•‡û6——@žð86Ó&¿ßŽ8	¿ç?Î)̵®¿åò.XŸ¡¿ë{ùJ¯&AGNfsrqGB6 J1604+5714?ïíhæŸ.c?_?0ù%B×?b—`ќ]?_?0ù%BÔ?ïlñòJŽ-?™d0ÿSË?'aÁ¶®:|?™d0ÿSÊ?í5‡z†Ä
?¤ƒŸE'	È?¶SÄ+Éߔ?¤ƒŸE'	É?îâ–orÖ?•õ…Ë,–?¡ß6™Ґ?•õ…Ë,–3FGL J1606.1+5630@U̚ÑVŸ@Fdä`gHäÀ:~À?öÀ;ë¼Õ±À $rÑç@Þè<k?ÿ'N^²½Ø¿ã«;þ'sŽ¿èbÅ'øþ•¿ÜÄò]€
׿ǯLý£sAGNbllRBS 1558?ïÿ¼œ†?]Oc3?ü(loG"?]Oc3f?ïÎh¸Ô?ŠÙ·•·•@?xþþK£•ñ?ŠÙ·•·•A?ïĄð›ÎÊ?+[1­¬c?}½‡²šÆ?+[1­¬\?ïÿì9ñnå>ïŒ÷j#O>ãÆ'Ö>ïŒ÷j#W3FGL J1607.0+1551@=`A€ÓÏö@Eµëž*ùÀ8kğס<À;]_Âví?꘴îDýÇ@çL‡`\@F¤‹¿á—:2›¿äE0X.ã¿äñšÃ‡¡¿æB7Š°ÈŠAGNfsrq4C +15.54?ïˆ|
–£?'~†'žé³?àüšX–ð?'~†'žé³?窕Ô?ÉèjXJ?ЫþÔWÉ÷?ÉèjXK?î	Eí‰Ò¦? ò'¤­/??¯k¡'bÕ§? ò'¤­/??áHf¿Ö³?¼»]4­Ð?Ýo3ò€R›?¼»]4­Ñ3FGL J1607.9-2040@v, <K
@6""?À9½¼{À;bYG™ò…¿'0ÖÔcø)@
c-ÜÝ<@?©c;¿Í2=¨4ō¿àæNè订¿ØØ©òçz¿ã²öЉùFAGNbcuNVSS J160756-203942?ï݇Ù<ü?s£¢Ç7?q<p"a¹?s£¢Ç:?ﭚ9©»?‡CŠ?"™q¼Õ'[?‡CŠ?ï:ROIû?'8Sâýêy?˜µ¼vÀ†?'8Sâýê|?ï0k¹òÎñ?‹k›ò_?™òˆÁ¦"?‹k›ò_3FGL J1608.6+1029@7ÿ·ä@Dh _ñØÀ8‡ôafLeÀ;\¤£¸×M?ôXO´HG@_óWûêr@óÑ@yí­¿æˆ{QZÁ¿æû…å\»˜¿ë	Jƒu¿í¯|¯AGNfsrq4C +10.45?ïßNªš`µ?léu!,^?pXª²Ï¥a?léu!,Y?ï5"Ië7?¡V\áÈÎ?œ9Mv™?¡V\áÈÎ?îb½}Jû?Ÿò½:‰ì?®Ô(+Pa?Ÿò½:‰î?ì¢â 'â?©4á+-TU?ºèï†þÀñ?©4á+-TU3FGL J1610.6-3956@u3¸Ÿƒ¾f@ þ{ßõH—À9ä@†ØÍÀ;
þ®Ç(?Û>ëÙÛ@(¬~¨@áé€aº/¿çþöjªï¿ét¢ #¿æZ||¨¿ë§"÷ 2zAGNfsrqPMN J1610-3958?ìP–±ûg?»‹íÎüJ?½{JwÈ$À?»‹íÎüJ?ì‡)£­op?ÃæïUYÖf?»Æ²â""ƒ?ÃæïUYÖf?çÍ@¥4¤9?¶Rjڇ€?Ðe~µ–·Ž?¶Rjڇ€?è³ú…=ïS?²2í^:­?Í0ëB·?²2í^:­3FGL J1610.8-6649@t™÷LÀ&J§€âéoÀ8[#'Õ€À:ìHŒ`Ì?êm¹'~[6@¤­ùwû?ü^¶­yö¿ÜxŸ
Î2¿ÔwFÀP4¿Ú»¼œpR¿Ñ3þÜáº<AGNbllPMN J1610-6649?ïçÒùq¶ñ?h¾Pèê¬M?h-ŽI4?h¾Pèê¬Q?ï+‡¡'h?§X;ì"?ºϲú?§X;ì"?ï0·x0º"?'v~ò'N?™éùè­½?'v~ò'N?îpqEA‰?™_¾ø…»?¨øë«î—b?™_¾ø…»3FGL J1612.4-3100@u¥ 8L@-JÄ!, rÀ9ÌÎFImÀ;—A¥Ãt?öCÞâ# A@"1jÜí?èÆ£É&Ð?ïýϘÑj
¿·l'ðû!Á¿ãÊ"Cñò¿åàÜ+íøAGNbcuNVSS J161219-305937?ê-ŠŽ$dâ?ÒN¼ö(.?ÇIÕÇnlw?ÒN¼ö(.?á]f7*}?ÖjÞ—¼»?ÝDß3'«?ÖjÞ—¼»?â­
;SŒk?¹Çî¶%°?Ú¥å‰Xç*?¹Çî¶%°?Þx;¬ë²?ÁÑÕÕ8?àÃâ)Š9'?ÁÑÕÕ83FGL J1613.8+3410@KŽÀA¤@G,|?ìÀ9…'Uþ9VÀ;ۛárv?¿¯½_ïð7@.ƒíŠÝi@Кßê¶Ã¿è$¤ˆœ,'¿áÂÓþüR¿æÎPZ‹¿ÜÌñõ-xAGNfsrqOS 319?ïlp<®y?˜xzf|P?'qý˜j0ø?˜xzf|PŽ?î¾Cל‹½?ª¦-Gë8?¤†7DC?ª¦-Gë8?›á*?£/i¦§è?¯E6Aía?£/i¦§é?îÌ¿×!Z?˜¼}ÃÐ?£>čêw?˜¼}ÃÒ3FGL J1614.5-2231@v	ÄupÅ@42«@‹
‹À8z½ø³oÀ;;…Ÿç't@Bv½K¥p@&©fÁ*,?ò˜(Ë{>?™È—«OF¿ÅPVHzÜÚ¿å³ìí\[Ü°×PSRPSRPSR J1614-2230?UNq²_ו?N.RjêL?ïõXÇ&Ð?N.RjêM?qÚußü?},YÁ싆?ïÜKAÒ?},YÁ싆?…bzb	?'>扒'?﫲v¾x?'>扒˜?b¸R²MKî?VþšÛ"Y?ïíG­M²´?VþšÛ"Z3FGL J1615.3-5146e@tº£3v¿å‰€5´1À6ï¸GʐÀ9»–~\&r?ï$&O­@þ°³¼…'?ýÔ]àZô?ïýßÉÿ'ó?"¬'ßZö¿à'7'߿ހ¡{j×OTHERspp?í$'&®P?¸þ›îÌ~?¶Ûoöʍ{?¸þ›îÌ~ ?ÜS_C|\?ÖvGãQ0D?áÖP^AÒ?ÖvGãQ0C?æ½}RMYà?µHdl?҅[eL??µHdl?曦—œ]?ÆU9`$T?ÒȳâÐÇF?ÆU9`$T3FGL J1615.8+4712@RwïÝëÙ@FË/¿á+ÿÀ:X¤ï81 À;ìGJAl²¿Ë•ÌŸDB>@@q@)ªo÷µ?ïÙÖɔ£¿áòT"¿ÜÚòaSN~¿å=†uûYÓAGNfsrqTXS 1614+473?ïúZ±™!?P1ݔQ?F•9›Ó|é?P1ݔ\?ïŽ:'$?˜vÕa܊°?HX¯»_?˜vÕa܊¯?ïdõëæݙ?ŽbÈ×Ú?"aBƒ$Lû?ŽbÈ×Û?ïÄêÓFi?t†,¯ãñ4?}þ
–\Ër?t†,¯ãñ:3FGL J1616.2-5054e@tÅـo&)¿ÀÈßK³À6"`4óþÀ9ákÀB{?·ä»uÊM@ÖSI3¦@(ˆ!ö¿áí¢F¼¿æ‰u_'®¿ãg–²^Œ}¿ÝÄ&¤`OTHERPWNHESS J1616-508?îzPiå?³OµŽ"þB?¨Zø	oqª?³OµŽ"þB?ê£>Î>Ô?Ð	|'9¥í?ÅsÇð²?Ð	|'9¥í?é^`b(ä˜?².ôjð?ʆ~w\m¡?².ôjð?ïìë/¡ð?m™uè'Ò?cìÐ^Ý?m™uè'Ó3FGL J1616.4+4631@R7Ã_Ñ ï@FÈûÿÀ? À:=aŠQþÀ;סS¢>"?Ù©¹‹Á-¡@­N€@­@»0à¿éaˆcÄÔ¿ê«ËŽå¿ä֌]é6²¿ïÿس"smAGNfsrqMG4 J161600+4632?ïþ'õve?.@¹'ìô?&Шži¯Î?.@¹'í8?í÷×Ëñ"?²Zv쀵¥?°AA§xvõ?²Zv쀵¥?ï'ÑgL4€?"WÇ\D?‹‹¦,òà-?"WÇ\D?샜ƒÅ?ª·c‹'M?»ãç×à?ª·c‹'M3FGL J1616.8+4111@PP9ßõž}@F÷¹¿©Î›À:"~êÁªZÀ<o%QÉ ?Ùf¯"ù>@Ù§b/'@ ™`
Ü·¿ã—"%ĵ§¿âP'gñ׿移*'¾¿ïÿWZýAGNbllB3 1615+412?äÛXJ­³…?Òõ¨[>C?ÖIOj¤˜ö?Òõ¨[>C?çÜpòv`?ËȎiÁÏN?ÑòG@?ËȎiÁÏN?é‹XÑáˆü?·£K;z¥?ÉҜ¸yÜ?·£K;z¥?å+°•¸®	?Á£˜ˆ`?Õ¨žÔŽ£í?Á£˜ˆ`3FGL J1616.8-2300@v	é€,
J@3w›ßÄ÷À9¼6YX`êÀ;73Ëßg?ìN¼9'Ùó@:zÅnÇ@Ûÿo·H?ïŠ3•XÂ9¿çŠ"ƒÉy¿Å7&‡ÔQ¿ïÿæPlOTHERglcM80?î2rÉ\ñ?¸¢õ/_ô·?¨ØÓj0ø?¸¢õ/_ô·?èÄ/B¹ÿ"?ÐY@ƒuƒ?ÌïBõ¬?ÐY@ƒuƒ?å³jº€OÎ?¶Tˆ¿ìg?ԙ*Šÿ`d?¶Tˆ¿ìg?çÉö+`Kæ?ÂfïðRï?Ðl©?h3?ÂfïðRï3FGL J1617.3-2519@uî{¿"ÿ&@1Î9ßõž}À9(>Œ,ɍÀ;ç½f?ïÜÙ¤ƒ@
Þô¾@¹³ ©BÚ¿ã¥æÞ4Âï¿ê³'ɮƿåOI¥v®¿ïß²Ej æAGNbcuPMN J1617-2537?ÛýM†ÎT2?Êåî®ÿ½?âY<˜Õç?Êåî®ÿ½?Ü(œ¼À?Ь'NÛÉ%?áë±ôt! ?Ь'NÛÉ%?â©ÆÖj«?·E"Û'Ý?Ú¬rÞS*©?·E"Û'Ý?Ç/M¸ü¶?¬ã´å2v4?ê4,'ÀÒz?¬ã´å2v43FGL J1617.4-5846@tp/hیÀ'ò€¯ËÀ8pº¼ÿÐ/À;I]A#·?Þª¶þÀv@n'!€-b@Þæ …Üx¿å÷ŽÔ'É¿èb¤‰ýè¿æ¶òI¿ï"äå-§êAGNfsrqMRC 1613-586?ïØi>^:?püVÚ÷¦Í?súK`Ðãt?püVÚ÷¦Ì?îqWx?·ƒÏ¡ž%g?®¸êˆ~>ë?·ƒÏ¡ž%h?î/G·Bk?  îhð_b?­¤‹ÙC?  îhð_b?ïB²ÿ"ð"?‹¼Ü!zÛ?—© 
aïž?‹¼Ü!zÛ3FGL J1617.7-7717@s–¿šÏúÀ2Ûú Âî'À8ª$[ÿÛÀ;b!¯é?÷whlP
Y@m¼Æð?@LŒX¦¿âËo2F¿çFMqj,¿ëϋó¿íA1×8AGNfsrqPKS 1610-77?ïª #R5?ì
œgº?…w÷;kr'?ì
œgº?裡9ÇÃ?¨?Bi#ؗ?œë
øǶ?¨?Bi#ؗ?î$ÃÜò=º? ÕZŠì#?­³Â0Ü$]? ÕZŠì&?ìYëBÄôw?¯mzxÎD?½0¥éØ\<?¯mzxÎD3FGL J1617.8+5137@Sûݿη‰@F>'_ÀYøÀ9ÈÉu)wÉÀ;ýåÑ÷?åÏòª""B@‰Ð2
@—'ÀŽP¿æˆAÁ!¿é¿˜ð°¿ïÛÛ3©
?ékpˆB AGNfsrqTXS 1616+517?ïÿFùØ	î?"Ý/÷YY? ÄþÂ2á?"Ý/÷YÐ?ﶜf@Ú?Á/Ptwk?'zæoÉÛ?Á/Ptwi?ïs²¼Z»"?ŠU	:Wφ?'‰¨t¨Ñ?ŠU	:Wυ?ïû|îæ´?RØõjíb?BDe/Õ±?RØõjín3FGL J1620.8-4928@tÞUùµc?Ø°ä_¡·\À6o'£+ÓÀ9·i$†È@þÊéG×°@
*Õô"»3?ÿ´>%–c¿Íóê:zG¿ß7åKÁ¿âƲ†@¿ëÈMt…–‹PSRPSRPSR J1620-4927?DºÅ ø¡?A©SDW?ïúÑN—؁?A©SDW?#©RÐÙ§?;ŠQ,©¬=?ïþÏEjÒò?;ŠQ,©¬=?xuTàðà[?u{«×«ä¤?ïÏV>@?u{«×«ä¨?4ÈßoºÈ?1óÉêá;h?ïýfä¿?1óÉêá;h3FGL J1621.1-2331@v'Àa"@2fþ?5ŸõÀ9*Et~WÀ;+Ÿé>ó[?úxÏ>ìúÀ@:Lj'Ä8@¥e;C"¿Þ¶a$vñ"¿éÆ»£"©ó¿ì¸ï6übß¿ÞÒ¶õä·êAGNagnPKS 1617-235?éYÚu†ƒ¦?Æ°·—°?ʘ–)åñj?Æ°·—°?êc*#ÿž?Ð¥5%˜Ô?ÆsWƒp‡?Ð¥5%˜Ô?æέêuÍq?µrÌ:½?z?Òb¤+e ?µrÌ:½?z?ÇòÊ6œrB?¼g:ÇÕÜÙ?êMrXão?¼g:ÇÕÜØ3FGL J1622.9-0312@%"¿ª¥[@>¶ÌŸóPÀ9PAÌS*IÀ;cÊõ\8?ê ¨ÍFÍÍ@
Ãt±­·‰@ß@QSÛ¿Éxà^*X¿æ4ˆ1ߘy¿Ýx(ïý\¿ìâ.w¦nƒPSRpsrPSR J1622-03?åIþ\Ñ>Í?ǀwäßÏ?ÕlF]'e?ǀwäßÏ?à77ì*?Ñ 	lª€?ß͑'«Ê?Ñ 	lª€?ãó"Rä×$?º%Še¿?Ø»Z6Q·?º%Še¿?Öù_w-?·îL©!êŠ?äƒPD?9j?·îL©!ê‹3FGL J1625.0+5651@U¦J`"@EÿÝÑÀ:•é ÀièÀ<­2ӑ㿷@X»§S@"x´q·'@+¾aO?ïýØ¢1Ýb¿ê«»ú¹çd¿àgªÝtöÞ¿ç³Îߪ'ºAGNbllSBS 1623+569?ïü`¢Zь?JQ#ý…Pi?<úí)s§Â?JQ#ý…Pz?îÆ|1—:%?¬®.‹ù²Ø?£˜<æŒ]´?¬®.‹ù²Ø?î9v·^ÙI?¢vSÀ<4?¬h"Šks?¢vSÀ<4?î¥2Ÿ"ßÈ?›"e2ùqÝ?¥¬Ö
Ò‡?›"e2ùqÝ3FGL J1625.7-2527@vP +"@0Ri¿·:"À6ñ\°Úþ¿À:u6xbm@O( °z@ðõ£ÒM@ÑBG£,À¿ßVàßØ¿å!¥øÞ´½¿æKf©¾f¿è«ÁYŸðAGNfsrqPKS 1622-253?ï®Ôö©‰ï?ÇÍB…kˆ?"JÂUƒÕ?ÇÍB…k…?ïËP""Å?'9ã^?—è?z~W?'9ã^?—è?ì7Çȸ*?©ƒZºÄté?¾AÁ¿>³?©ƒZºÄtè?ïêõµâ?j½f 'Ù?e
ðJí1?j½f 'Ù3FGL J1625.9+4125@Pa¾À//˜@F@`B_÷À9Õ¢"›À;Îï@4£¿Ïk¶g/º@'G¡)Zí@›ŠË<T¿äoG¬DŸ ¿éÔìò9Ì]¿â›i+Mò¸¿ïùÿ•¡èHAGNfsrqB3 1624+414?ïü`ZíäÉ?BQÆëFô?<ý(Ù´?BQÆëFæ?î¢="ýX?«OWT°€?¥Ü#Ö°*|?«OWT°?ï™/0ê·?…¼ÕMja¥?‰½43ÅR6?…¼ÕMja?ïATí.x£?M"Œ?—ÕbZ0ë™?M"‰3FGL J1626.0-2951@uÌó S\ž@*¢:Þù;À8>þ½	á*À:×Eßaô?÷¦g½ÿT‰@ Wš»-@IA½d¤ð¿ÜÕäÎ _¿è' +ø	¿äˆ=H,a¿ï	â.*W9AGNFSRQPKS 1622-29?îÜQUÌ·C?¥DøísH?¢:ê£4‹Ì?¥DøísH?äÇ̂ ?Îî"mgø?Öpfú¿Çè?Îî"mgù?蜽9ž*g?²U
|îÇ?͍‡Vd?²U
|îÇ?Õ։VÎúJ?³ÅÏÁžúÃ?å»T˜'Ü?³ÅÏÁžúÃ3FGL J1626.1+3512@Lr"_õI@EôŸëWÒÀ:ۃ6€ÅÀ;ôyŽaW3¿èb‡Žv8@|¼êº?û2ýáAÎ׿ïÿ2Ìʸ9?ïýíXTø!¿Âs,·1ô´¿àÅÙ=žqAGNbllRGB J1626+352?ïþ†Á?,Åqo܁?'ž3î^ú?,ÅqoÜ´?ï¥cúõØK?"ï ¢?†§B‰ík?"ï £?ï{{T8	Á?Š±µC?à?•xþÇï?Š±µC?â?ïóú]˜°ë?\Þ¢u2<?XDΞ*8?\Þ¢u2F3FGL J1626.4-7640@s¤*ÿójÆÀ2Î_¿ƒ8.À9ÜKŸ:ÃJÀ;'"e'¿ùS)ÃGèÍ@+è«ûpú?ÿØJ^Èã3¿éI4'ª-¿ÔNd8Üü¿â‹&9O­¿×òÕÒ|["AGNbcuPKS 1619-765?ïûÅg¥ì?;•$ÔKkù?@êahOú4?;•$ÔKkì?ïØköpíá?p2<…v?sÊlj?p2<…x?ﴎbíè?€AœöhB?'Ü~gD†?€AœöhC?ïÿ}³s?¾#î4?\?i'hA?¾#î5b3FGL J1628.0-3203@u·(€QÉ÷@'½ ‡_À9"éû±¼¦À;<êºô]5?û"á·©°@a&xº¦Ú?û ¤†_¿ÀñÒQ{Y¿Þ‹·½"k¿ë"Ú±¿ïÿexª¶¢PSRpsrPSR J1628-3205?fh˜r?lÖ˜5§Š?ïé—gôàó?lÖ˜5§‰?tߕ*¨GŠ?";§¦sñ{?ïÖ@Õª¯q?";§¦sñ{?Ÿìxz)l?—1c•jo€?ïœ<.´ ?—1c•jo€?‡9´þ.X?pܤ<‰ï?,F?pܤ<‰ï3FGL J1628.2+7703@[×6&-@A(?º*3À:†±Ö§A"À<bf&¥†À‹@€MÃ,@Í¡²—ÂT@—Á_±@¿áàð|¬,¿ç`Çk¿åšãˆG"¿â3 C+ù®AGNbcu6C B163030.4+771303?ïàäÉÆí*?ˆNe˜øD?o69Ղ?ˆNe˜øD?ïÙûN†€%?~Y 9fP‡?sX¼¿în?~Y 9fP…?îÓO/{õ¦?6¦úÕ?¢Ë
@¥"?6¦úÕ?ïÿÒ¨eà?ÉÚ=ù1>ö«üÍÈ´?ÉÚ=ù0Ü3FGL J1628.9-4852@tô	`0Â@¿Â±Ð ƒÀ8#ÙìpCÀ9ð¿UK?ø/L>h@ÝéÀ"š_?ùw/É~?ïù•‹–¢¿â3,}6¿ç…sq礿îA¼}Ê0:OTHERspp?EŠ®ÆÀÔg?L3—lˆgs?ïúTNOË?L3—lˆgs?Z>0ˆ-µƒ?o©þá¬'Í?ïòàç»é%?o©þá¬'Í?–‡xüÇùc?'Ç#æ?ïKÄ8À5?'Ç#è?£ËNº"ï?—;Rk0Œž?îÃK_}Ñ?—;Rk0Œž3FGL J1630.2+3733@NŸ C×Æ@E¥IÿþRÀ9´ s¨nIÀ;Ÿ0¡ˆ{d?úxuz*"|@©°Û.d?ôÅ›À?Þ,ôæØwâ¿Ü£9~Y׿àl³Ã¢'οïÿëÙ¾ˆøPSRPSRPSR J1630+3734?•ý†­åEB?ô®,º?ïPʐÕÕ?ô®,º?–!L¹É!r?­wÖ|?ïNõš1¶õ?­wÖ|?ºÄ¨g"?¬—ѳcT?쿧}ªó
?¬—ѳcW? ²2—«?—ϲ®{6Î?îôÜ֎~†?—ϲ®{6Î3FGL J1630.6+8232@\ó(^ÃÚ¶@?@*@EjmÀ9<¿"ÀiÀ;¹½îãx
?ö*6ÊÂ[…@I¬3$E?þ9[-£&`¿ÒmOÄcq¿¿å¶3ƒ:2¿ä|1Ën™¿çÜŒ{›AGNrdgNGC 6251?ÚÖÒÇá˜?ÉÚÆÓU;?â"ô–œ4?ÉÚÆÓU;?Ìùœ?Œ—;?ʾobM¶å?èÁ˜ðÚ2?ʾobM¶æ?ãGnúæò?µ²WžMw?Ùq#ú
2?µ²WžMx?ÃAuÿ—{–?°ÿŠ~ö¶v?ë/¢€!?°ÿŠ~ö¶v3FGL J1630.7+5222@TÒÿ" @E2_×ÖìÀ9?¡F6E6À;'úÀûÞ2?àáøÆ®XK@'uiŽŽú?ÿæü9¢¿àí7[¿w¿Ú#{£¬\¿á¬ž=1'¯¿ß6"›¹ë…AGNbllTXS 1629+524?ïúdEƒ=Œ?DœStñ'?Fnéó	Í?DœStñm?ïs¢p™ò[?"Þ²e'¢ß?'‹±ìÁ´ª?"Þ²e'¢Þ?ï+þúTC?‡ñXÿ?Œ5AjïU?‡ñXÿ?îåw"pµG?¨ÅÓÅÞ?¡¨†Èô«"?¨ÅÓÅÞ3FGL J1630.8+1047@:uxmži@B/ÿ¢/À9›ÉØ)øÀ;†™°?ÎL?ár'3Ô÷F@éFÅâ!ô@o¬ÙO¿â"¬5[47¿íÕ=}µ¿â6}g߸7¿åÙEìüË¡AGNbcuMG1 J163119+1051?ïúeŠ"?KZc*­n?FkµÕïéÞ?KZc*­n?îí½A'ý?¦ðçDGJ7?¡.D+æÐ4?¦ðçDGJ6?ï@€­«e?"µ·²öDë?œïêJ"5?"µ·²öDé?ë0ˆA@°–?¬eq3"?Ã=Þúý=¦?¬eq3"3FGL J1632.4-4820@uŸà·ö¿ÉA×ép-À8Bî'sÀ9æŸÐë??ø‹9L&õ@<öùñóù?ø5^ɹòÕ¿íù"ýW`?Óø/ª´ì¿åJ#ËÈQ#¿ê4zý2nPSRpsrPSR J1632-4818?Œ yK'‹Ú?®!#úÈßÐ?ï~ѵÒ?®!#úÈßÏ?"†ÚOBÚ?¡;e9ƒ?ï­ä–ÃÞô?¡;e9"?ºóÁ˜W>
?®Õ#ÿoâ?졇Ìõ>?®Õ#ÿoã?¶†Àœ»ê?©cAaw§?í/'ìh'½?©cAaw§3FGL J1633.0-4746e@uGñQç?¾ó@`å•hÀ6°\S½íÀ9aÓÚÞ?ç	÷¹EÃ@ì!´@â¯3+¦?¿§¾åi¿ãg´¯Ÿ•\¿ãvt€Û\³¿ã†.þE?ÐOTHERPWNHESS J1632-478?êÞvÎÜh?Å»F¾Ø¸é?Ć'ÐĎ`?Å»F¾Ø¸é?ݔRÔÙ³—?×?ƒ>5?á5֕"&5?×?ƒ>6?æPÑVœ¬&?¶ƒcH/<@?Ó^]RƧ´?¶ƒcH/<@?ç1['¸?Æíùœº:?ѝIÓÒú?Æíùœº:3FGL J1635.2+3809@NŽ?é$@E+uÞÝqÀ6°"T"—À:¬Ò['@ä–ü±A@z®ž@©š¶$>Ï¿á\¿Uڗ¿æۋV`Ë¿çË,æÃ¿ë+ômáÁAGNFSRQ4C +38.41?ïJ%æõø'?›ÇptöP?–»C!@íï?›ÇptöP?ï´²Fc?'@}›—e?'þ:"ng7?'@}›—e?ëuXŽ5."?¬[õ8Ëo?Â*Ç+E±?¬[õ8Ëo?ïúÚ¤íT?Pǽ%8´?D•oœJ°¢?Pǽ%8·3FGL J1636.2-4709c@ubŸœèÙ?ÀèÏÀOÄlÀ7f×süPÀ9‡ëÕ¦"?ô"Þ+ÄÔÜ@4ýOü@·˜?§_Ö¿çñ¡B…a¿å©î{s>¿ç¢8¤Œ;ã¿èW}?pÙ1OTHERsppt?'3LÕm?¨òI>R?ï·1ÂÏÀ«?¨òI>Q?´s–Að"Ï?»÷ñ˜™G_?íq7Áí‡?»÷ñ˜™G_?º¶"ÜÓ?²jEäÖN?ì©.¤ež?²jEäÖN?ÇÀfrU?¸Ú´9X?êû&cj?¸Ú´9X3FGL J1636.2-4734@u{à~í¿ÄC€³CºÀ6ä'eîqbÀ9'!àÄÑ@=ÃòI´@ž>ïÔå?ûC¼˜L=?­Müƒ"À¿â8¶)ó'¿ãþÒ–³5¿ìö( ­9OTHERsnrSNR G337.0-00.1@?5ÌwŒw?0€¼ZŒe?ïýFqq?0€¼ZŒe?1h³±yž?IªÕ+úDÃ?ïýÒ韩Ñ?IªÕ+úDÄ?s"4­CÖ®?c9å#"c\?ïØٖ¥xR?c9å#"cd?f°#¾^µ?_«
6?ïéOÜA¡å?_«
53FGL J1636.7+2624@Fßß´0@D€C‡>À:FوœòÀ;Ú´*>—ë?áfà•'µ
@ñ‡î'ð@Pbà?êøì#eq¿âÅAµ?¿×-ɀ«Ñ¿ãÊ*î7¢üAGNbcuNVSS J163651+262657?ïÛÍ'v^?y{NF?r}lDÐÑ?y{NE?î#˜àðv?®xyè´K?­Æqþ€øš?®xyè´K?ï;ˆK»?¼áb*?˜œŸÎöˆx?¼áb*?ëM¿šÄx??¯àð,œ?ÂÉ"î?¯àð,œ3FGL J1637.1+1314@=ÿ¥ßøù|@AÙÚÿ•võÀ:HNäi¡"À;›üD}Þ?ÇÇ9‹£@§ºu\M‰@Ä¿Àéz¿ì/죛"à¿è˜É:.Û¿ÃÐ'Ü}¿Ñħl¥ÎAGNbll1RXS J163717.1+131418?ïþc³?5%NB;îV?.	ÎoÔ½¦?5%NB;îZ?ï¨$º¾?™´ê|›F?…öûP~^?™´ê|›E?ï¡ÞóåHá?…8:qÍæÓ?‡ˆC­Ç—?…8:qÍæÐ?ï™ûΔå4?'‹2`Há?‰ZƲÃ?'‹2`Hà3FGL J1637.6-3449@u«•¿ðEx@ \îøœÀ9Qc"GÁÀ;"g¨…ŧ?ñWmû@
a–4à2?û¶¡>ÿo6¿ïÿ¿Ä.KK?ïÿ†ªBx¿ÛÓT"	•^¿Ò4>ñ'cÈAGNbcuNVSS J163750-344915?íøh¤ŠÍ£?¬2û3òd?°<ºÛ©'â?¬2û3òd?ì)êRUÌ?ÆõÑ ³ô?¾°¯ÍmQœ?ÆõÑ ³ô?ë)­TäÇé?«¡Bþáö?ÃYJ¬làZ?«¡Bþáö?ãaIòÀ?ÁÉ¥:5¿%?Ù×Å=l'?ÁÉ¥:5¿$3FGL J1637.7+4715@RYÉ`0Â@@DñCÀI0ËÀ8'滋[éÀ;ž{Àj¾»?äôÛìû@~@T7$Y{œ@ð°ÿç¬L¿ã{·¨<8"¿åæÞP$R¿ä
këØο谨Ýaø÷AGNfsrq4C +47.44?ïý4N¼‰Ô?8]^Ô@?6]Š±[Â?8]^Ô@?ァ B?Š¹c){>™?€¿ï\`?Š¹c){>™?ï 'wî6?ƒÎñ^e ?‡ö"8"r­?ƒÎñ^e#?ïþÚgÕ¹? @YujÈH?"Y¢¤bü? @YujÈE3FGL J1637.8+7325@Z~V>Ðö'@Aœé	:;À:è¢[ßú§À<<zØä2D¿¬'–°OÄ@ºðëeU?þ™é`+cÜ¿í]èK‹ø$¿¾­èlK¾Ö¿³a»Fg˜k¿çòג<rAGNbllRX J1637.9+7326?ï[ÂÁ´*?•Zª&N@0?ˆ©O'õZ?•Zª&N@0?ï˼¹|ü?£Œ/ë= ?œˆhÐ`{?£Œ/ë=¡?íK-C©?°ýà¿c?µ¦•â·§?°ýà¿e?ïM=["Xš?'ÉJû¬n_?–XT"ì¯?'ÉJû¬n]3FGL J1637.9+5719@U¨s¿ë<ú@D2Áð8À9ÎØuw{À;÷–uŸÀ

å@CsõÆN@p¸ßÚñ~¿êýiEÛ_¿æU¢å®×*¿ëñð¿åžo"r@AGNfsrqOS 562?ïÿ}±¼Ÿ?qÂnô'4?IÈoÌ>Å?qÂnô'£?ïÄ+g¯?Š‰ZkÒ?}óöjL)?Š‰ZkÑ?ï½ô'!?€¦p¨)?€ Û·¿i?€¦p¨*?ïÿïôQ,l>æéxòò$¿>à®Ó•â>æéxòò&Ô3FGL J1638.6-4654@uƀ"?u©`À7W=¼ùðòÀ9¥ýò߆
?þp뽨@g¹X%ÛÝ?ü·2Ü¡+3?Ç1i™÷k¿Ý÷áìåLjar¶¬¿ê*r.ñ…OTHERspp?ºTÕÔÎT?¿_̾'›k?ìµeEf?u?¿_̾'›k?‹v?2ø'?ŸfÙ´M#?ï"ò'4?ŸfÙ´M#?ÌPp×Àô1?·=çq¤Ç-?èëãÊÂô?·=çq¤Ç-?µ>s>—ÖV?§ØÖZ›Zµ?íX1˜-5?§ØÖZ›Zµ3FGL J1639.8+4125@PdzøÞ¤@DÎ3_¨ÝÀ: ¸jßrÀ;ÃiÔ¯ð?à›{'=™@"NAxÆ@UÀâcb¿ãõ×|B	ª¿æϐnw¬à¿è¦˜!ˆˆ¿ïýžIè½AGNfsrqMG4 J163918+4127?ïõK‰L:ë?Yo
¾?UhígŠ*å?Yo
¾?ì_˜.´'?¾§"y #?½>Š[ö?¾§"y #?ïlܺ°Kï?Šz¦™:Ù?'dh©ö''?Šz¦™:Ø?ènEŠÆ¬Ü?·
6ëû?ÎFéÔåL?·
6ëû3FGL J1640.4-4634c@u$_•'Í¿"'‹Ÿ«¸rÀ8Ø{,ÇÀ9Ñ)‹ê"n¿ö0	£—Ê@
jthÏ?ý»¯ÞÕbó?ì} ⣣´¿â:Áœíáð¿âNªRNm¿Ô½p"ý°ðOTHERspp ?êŠMøqÎ
?ÅJ¸'É?ÅÖÈ8ÇÙ?ÅJ¸'É?ìPj¦A1?Ì6µš¶?½{"ªÍöu?Ì6µš¶?è01–š¨?³k€µGþA?Ï?9¥Á•c?³k€µGþA?ïöt¡(P#?h¨õøI[?S½¯_¹8?h¨õøIa3FGL J1640.6+3945@O¬Xߕ&m@D²•ÿ±%§À8æ…Ûv´À:"+,Ôta?øãW/ç¤?@6€´yS@5­ƒCl¿ÐbÜXŒ¿å~¯´ý¼ó¿ãÝtŽ-î¿êY©1<8AGNFSRQNRAO 512?e*€=?$ER´Gx?‹Ufµ_ñJ?$ER´Gx?ï¹çú ?Í# §ë?†;¾ÁwÅ?Í# §ë?é'¶C_Ï>?¯G¹Ù©[?Ëa&ò€Ã?¯G¹Ù©[?ï¬ìu	 º?€Ï9Nè%?"Ä⽗ъ?€Ï9Nè$3FGL J1640.9+1142@<āŸ§Ð"@A–`)5ƒÀ:ÛeìÃãÀ;•ô©Š¨e¿âêz6Õn@Ív&wãç@]P¨¿äÌ®>0+¿æa†&(¿Ð­b…÷¿ëb$yµùAGNbcuTXS 1638+118?ïӕ´–·<?zéPK¨?v5%´¤b
?zéPK¨?ïBÝ:‰ãA?žž‹ÂøL?—¤X®Ã—Â?žž‹ÂøL?î½ÊbO?£©Ä19?¯´#YÛ»?£©Ä19?ïL,Ì?Žée5¡?‹ìôúLùÐ?Žée5Ÿ3FGL J1641.1-4619c@u(; îÙ?®æ»Ÿù'À7'œh€òÚÀ9›œÈù¶¿ÏcôçH#/@
ešO±™@:_¢Qú¿åPŸŠtb¨¿ë%nâO¿Úÿf}›¿æ|Í{Hu»OTHERspp$?çGs	·Ïý?ˇ%}~?Ñqì`?ˇ%}~?ä¹:¢‰Kf?Ö.\ÝL66?֍Šºíi3?Ö.\ÝL66?äYÿQÂÂm?¶zÉ8Ô0°?×L\z{%?¶zÉ8Ô0°?îÍù{+"?·ÊbÃôwÐ?®" hMFË?·ÊbÃôwÐ3FGL J1641.8-0619@%¤rAeûÝ@9ÅYa›À8ÍÎ8׋À:æÃr°÷"ÀëýT©û@ˋo_^_@†î_ċ¶?ߟ'
ÈÊ£¿äeún#QÇ¿ãEk5œÞ·¿áÊÞ:ˆgAGNbllTXS 1639-062?ïúô`UÂ?M•)õŸ|§?D.}¨û$?M•)õŸ|Ÿ?ïÞ&øÝɐ?{"Ö¤Øm?p샑7ã?{"Ö¤Øm?î€ÇuÉGF?œëòߕžç?§óˆ£k‹}?œëòߕžæ?ïÿӌvgÎ?ý½ÓO9ä>ö9ÄÌ…Ú?ý½ÓO9"3FGL J1642.9+3950@OÀÍ_™Ã‹@DyvÀP½ˆÀ8"è1­!À:Á͐A+C¿ôÁ}ÿ	_û@;64D€8@"H?ß¾í¿å֜ƒÑ'È¿åÃT±¹Õ¿æ0'êðñ'¿æ‹Z˜
8´AGNFSRQ3C 345?ïûX_Dj?M!]NO?Bžƒ–îVJ?M!]NJ?ïÅ8²s/™?Œ™îN?}c¦Æh2¸?Œ™îN?îízÜV¿à?™RϓéŒR?¡(R:"ý?™RϓéŒR?ïÿáã'>ý];O'}>îûùØÉ_>ý];O'|?3FGL J1643.6-0642@%"~e`­@8zE¿ý±qÀ9†ãOÆñÀ;…CÛ?™zVº@Ð@2*M±c»@'
 yó¿ìK1uT&.¿åw©Ò]'¿Ý|•DDº¿ÓÑýÀ¬ûCAGNbcuNVSS J164328-064619?ïô¯|›?eC¹Œå‰?V¡åôÆù?eC¹Œåˆü?ïÐÞ5r?Â`êzÄ?wõþåF›?Â`êzÄ?ï'ÑM?—LWëÉ?›…Ö]½‰?—LWëÊ?ïÌö‰"+?r«U•H:?y"»6}ê¨?r«U•H;3FGL J1645.2-5747@t£½ßÉÿ"À¨
`+8éÀ9–u—5À;Í#3᯿ör25J@
ÝeÌ7§@f+ —ºœ¿é7¤
zœ¿êäT®-${¿à.­i"¿ç^瘙ÙAGNbcuAT20G J164513-575122?ïô‡ÿRt?ZÞïŠÉ "?Vñþ[—?ZÞïŠÉ Š?ï=js-¢½?®ï£¯é/¯?˜R±šK¨?®ï£¯é/°?î§Â*b"£?šÝ	‹‹*í?¥ƒÝYÝÕ¤?šÝ	‹‹*î?ï÷ÌÝì?Q¾¿q0±j?PgÜE)v?Q¾¿q0±W3FGL J1645.9-5420@tÏß֔ÍÀ'`óÀ9?‰i ­ŠÀ:æÂ:¢"=?î¨JG³3@Ȗœº
}@¸€nz\¿ÛŒ8óf"Š¿ìŠ!n«¿é3BL«ª=¿ïþNh†ÒOTHERspp?Û·|ý,X?ÐEÚ§¿…ï?â$AséÕ?ÐEÚ§¿…ï?ì¡Åv&\?ÈêóÿÝ?ë׎¢vh?ÈêóÿÝ?áÏ©Š'[J?·IÔ#úÃÒ?Ü`¬ë±Ij?·IÔ#úÃÒ?Â{Û¦¨N?¯B¤y3‰?ëa	;VUí?¯B¤y3‰3FGL J1645.9+6336@W‹ž_Ñ÷¯@Bó©?ÿÊPÀ9ÑaE•5‡À<5ŽWF8¿íÍ2Ñhà@kC¡•f"@|/@_k ¿æö~b—µû¿éÆVv·Êæ¿æ_o¯:jµ¿ê'æ½õՖAGNfsrqTXS 1645+635?ïÿµ0mÓÛ?½ý0©?³ä‹	Fg?½ý0©¾?ïÉE°x©?ƒ¶[ýJi?{]'õC«7?ƒ¶[ýJi
?ï҃ƒg!?wÏUZ¾´?v¾}¾Ln¸?wÏUZ¾²?ïýÈۂ–?1ä/Pæ`¾?1¹#ëO:?1ä/Pæ`Ç3FGL J1647.1-6438@tOÞ²gÇÀ(Þg@€ùÀ9»†ÜþsÀ;•BâL'ÀxwRœÚí@Þ
ô¸@ƒÄ`Á
¿Ü€Õ$V˜à¿å.ߥRƈ¿ã½Kõ÷¾h¿Ýÿ¦ù¬ÕAGNbcuPMN J1647-6437?ïþuâNKÁ?,*£ ?(¡ÛCó-?,*£ ¿?ïÔõËP?‰¬—c³?u…~WþÑ?‰¬—c³?ï£3ºø"â?‡ã‰ØþÃ?‡3AÞÇË?‡ã‰ØþÄ?ïÿýž™>Ä1	ë
¢>³3:ü1>Ä1	ë'Þ3FGL J1647.4+4950@S)®_ú;›@DvŸ™ÛÀ8¢ßüTÀ;±m«Õ€?ëO§Á‹·?@<yX@nÈáÉ¿ä»ôbgÿ¿æüÓ¦8l¿æ"ÑËAæ¿äð滜‰õAGNbcuSBS 1646+499?ïý¾ë<ˆ?/§
w»p?2€¦ž?/§
w»=?ï\ Šº¶é?™Ü>z­‰r?"{"É?™Ü>z­‰p?Ö{˜—?…|Ógt"?ŽPJaÚ:?…|Ógt‰?îj<Nþ}?š¶ÇZ‡™A?©^|;7?š¶ÇZ‡™A3FGL J1648.3-4611@u6òä¼®¿é©Ùà(ÀÀ7ü¼b~À9íý©
ªã?ý#íãr֌@½•6Þcx?õ:7>/»"?ïò¦æ‰6u¿ÁIYvz¿ÞSªL^¿í‹9Ëím›PSRPSRPSR J1648-4611?LÇ[‡Aì?O?^NçŒ?ïøÎ;i/?O?^NçŒ?NY+öÓ-?h©sa}N?ïøiµK6?h©sa}N?¡\n~V¢?žÿÊKëœõ?îïê9–?žÿÊKëœõ?5ÒÚd"?"+ÔΚ?ï‹(´–oÓ?"+ÔΚ3FGL J1648.5-4829@u-••ÀxNß·
CÀ8»
Z[–)À:m‰;}…?ΨÃ:VO@	R|N°@N wm?écØÏ[꯿î,™¥qØÏ¿ÓXå~
eÞ¿ã%ö 'AGNbcuPMN J1648-4826?ïæœk½?ªÅìuð?žƒ,}2ˆw?ªÅìuñ?íÜÌ`IJ?¼l–O]?±œýµ¯?¼l–O]?ê ü»kd?°­$+C²?Ç€
Ro?°­$+C²?ïYÖxæœe?"~;*^k?"Å0ã,sq?"~;*^l3FGL J1649.4+5238@T}òÿf@CÃÙ?¡ÖÀ9'm;l¾À;ÙuxR!5?ïdí·ËUK@@¸Í'n@À@Že‰¿Õiïk¿áp&ÛèÛ¿å©
O…
¿ç½LþµyAGNbll87GB 164812.2+524023?îéï]cÇ?¨xCâ–áV?¡o
)Í?¨xCâ–áV?í.OEÝÝ?µ§ŠŒrÊ?¶…Ñ¿?µ§ŠŒrÊ?ìB—
¨ ?«åæñ[?½ëG'¿??«åæñ[?çD\/•°?³mk¸4åó?ÑwGû Ô¡?³mk¸4åó3FGL J1650.2-5044@u.ŸðË°À«ÎÀAùõÀ7©ZÎyÀ:©6»}ïð?ÓÐӆi)ÿ@Ÿ,¾O¢@]'ßæÚë¿ä÷*JY¿æMc¡ÅÍ¿âÎÖ£vx¿ãZ/ðCۈAGNbcuPMN J1650-5044?ïú¯UÉ»Ñ?L´D½Ñ?EB¨Ùº?L´D½Ñ?ïF`f=¬?¨1­,gŸ?—3ó8J|#?¨1­,g ?î.^;X0á?¡mÃÃiÏ?­J|ñæ?¡mÃÃiÒ?ïù.3–?Fc§ìã™?K»G³1§ò?Fc§ìã›3FGL J1650.8+0830@:œò?Mé@>¢	Às"7À9lž#lÓÀ;nâO?ä~Oz!ëH@¢€Èè<@FÀ—ŠK¿åø~¡+H¿é§ÅËô<¿äIFɤ4Ž¿ïÿi¢¹†AGNfsrqMG1 J165034+0824?ïùíoK5B?Jä~ýÒ?HJBÓ*ûX?Jä~ýî?î ™ڗy?¨ªêeµ!?­öoBVˆ~?¨ªêeµ!?ïðÔZ¹E?•ÍìëÖï?œåt¨×7?•ÍìëÖî?é×.C<£?­›X/ßѼ?È£Fó
s¯?­›X/ßÑ»3FGL J1651.6+7219@Z³¿µ@AZ–`)5ƒÀ:ÌÄbšÿËÀ<$#wÔLô?Ö.u{N¢G@
êO²¥"?üÍ+4¾y¿ç5Œåj¿ÞR´úw뿳d™ûœÌˆ¿ÙÕ~5©É×AGNbllRX J1651.6+7218?íڊ‡¿>?½Œ=™â?±+«Çê?½Œ=™á?響Dàü®?±-ç<?…nÇÀԖ?±-ç9?íÿÚcuï»?¬²_ü+Íz?°,äP')?¬²_ü+Í{?ï*'F¹Ÿ?'›$Á÷t
?ˆµ[nQ˜P?'›$Á÷t3FGL J1653.9+3945@OËôàM/@ClصýÀ6ÃðÈT˜À:(3Auì¿òBªפ—@ø|¨òþ?ûv'¿aª?¿×Ò9M¿ÜU,Ò,C¿ÒϰōÆÛ¿Ó%°)d8 AGNBLLMkn 501?ïëžêµé'?l*m'+xÍ?daJ}Å?l*m'+xÑ?ïÀÛ¤=¤º?Á®'á"<?'-á-¢ ?Á®'á"<?ï[,;¥ß?œÖ¯ÿýΧ?žtšx‹DU?œÖ¯ÿýΨ?ïÿùvl—ß>Ù"£ŠVî>Ê&M ƒ'o>Ù"£ŠaI3FGL J1656.0+2044@DDãõhÍ@A"'@	‹À9¿å¯ò¡sÀ;±b'¬K¿Å·zº9ñ@üZNU"œ@ñaÿÏX˜¿ãi Æxd¿è%/u5)¿á¬@ÒFøý¿å '<9ÁAGNbcuMG2 J165546+2043?ïÿÖÃì3ù>÷!eæϙ>ôž	æmn>÷!eæÒ}?ïҔœ¶H?.Å%XÞ?vµ±¤Û·q?.Å%Xà?ïáÞ8˜6:?q	¦H@‰?n!ÇgÉÅØ?q	¦H@}?ïî¨aAx?X$²68È?aWž¾‡ê_?X$²68¾3FGL J1656.2-3303@uépÀ&Ì@`™?׆dÀ8Rys‡À:æ#wÔLô?sÒ­@³ožss@9·?œÎ¿çšç{¾¿éõÉß÷;¿ìŠ?£GÜý¿ïÿˆs¬uAGNfsrqSwift J1656.3-3302?ïù†~ˆ€?PÜ+ÍÅ,&?Iç²ÞÃ?PÜ+ÍÅ,+?ï9}#ôS›?¨;¬ÃºÞô?˜Ð[uŒm?¨;¬ÃºÞô?홠´Š1?¤¶PÆӑ?³2ú[¯Î{?¤¶PÆӑ?î*ÝhH+"?šŽâ8w0?­R){}MØ?šŽâ8w/3FGL J1656.8-2010?ñŒlà@,%8@¹-´À97
ðôÊBÀ;/[àÑf?ô²Ãú@Mx@òûûcŽ?ÿ`%ßãí?ïÿ›BÞnW¿Û9'lIF¿àÿ£¿é׫»¸°êAGNbcu1RXS J165655.0-201049?¼¢Ôb"Fü?»œ×À?ìk¥s­w ?»œ×À?Óôa™Oë?ÐFê½²©?æÏ3yØ?ÐFê½²©?ÄbA×*?¶ôå6¶?êü'oŠ5{?¶ôå6µ?Ð+H$ôË?±Œk«®Ñ?çê}[텚?±Œk«®Ñ3FGL J1656.9+6008@VbøÌN"@Bµ²€l"À9Û²~líÀ<ÇC ¿Ð÷Q¼qq@'¹E†qõ@ûkŸ¶>@¿å eJT…¿è"²ÉF¿ç©ó_n᛿àßZYAGNfsrq87GB 165604.4+601702?ïû\­ ïÌ?TÐþÒïx,?BI|@Õ?TÐþÒïx,?ïs4?^?•{Hg}T?ˆ¸ã2ð(g?•{Hg}T?ï¹ $¶p?ƒ•©"39?·ù6Òd7?ƒ•©"36?ïÇóÄô•
?u1Òv°ð?|…µyù?u1Òv°ï3FGL J1657.7+4807@R–»À5Ö@C>'ŸÐ€À8¥Þzt:dÀ;³r–'–?×Ü$÷ŽÊç@\z–9ý@ÍÖ©˜¿ä…ˆõ lÌ¿çEȊ"(¿æâ°ä0c¿âcóü«P•AGNfsrq4C +48.41?ïÿð[?A»_ó?áôž@5?A»_k?ïÁìÔ¾>m?ˆWÅÐ-Þ¨?	• àÈÞ?ˆWÅÐ-Þ©?ïÍßSOÈð?w²¶`«(?yVX‡Þ?w²¶`«1?ïûÃxb†"?;ad>¸Q¡?@òuå¹c?;ad>¸Qˆ3FGL J1658.3+6149@VåT¿àU@@Bwìàh‹À:•€,
JÀ< œé°2b¿èl?Dþ%¤@¢A]îH@:»?†¨¦¿ê"Õ0.Ø¿ÜðÙ",¿ÛK€:;Õ¿Ö:µ-+AGNbllNVSS J165808+615001?ï[rqÌÎh?¤>ºŸÂ?"'±Æf3?¤>ºŸÂ?ï¡É[ïBë?")Àá}K?‡©/E?")Àá}K?îzøÌæ?¨£¤o–:?¨^Às?­?¨£¤o–:
?ï䍧Há?ho1çòû:?krXo· î?ho1çòû<3FGL J1658.4-5323@tíÏàGÓÔÀcð@uÀ8ž•Ï	½ïÀ:ðàŸèh4?þ-µÛC³@
¶tñ™‹?þó`Åg¨±¿à_Âáø"7¿á¥v»¿êù"iiü¿îÂi'¶ºMPSRPSRPSR J1658-5324?1#P¨4ZŠ?0¯sãŠT8?ïýەêùt?0¯sãŠT8?YYùƒÐ'?"¯À°6×?ïóS>·?"¯À°6×?"â
}dÜÕ?Œ
Ï	Ì<‰?ïXï¬Ù?Œ
Ï	Ì<?_âb[A–?N]çðž2·?ïðÎÒv_?N]çðž2¸3FGL J1659.4+2631@Gŝ¿™£@A¢¼ßï¿@À:Lyãñ¬€À;¾†ß'±÷?×ýißäùâ@ΔY=ÞÞ@­–@ž«§¿çeXøŸ¿äKÛyý‹Ë¿é³_
|…¸¿ØÙ,¸V~AGNfsrq4C +26.51?ï¸ÁÖ½'?ˆ"ävOç?ÿϊPŸl?ˆ"ävOæ?ïÆÀ£Ë??§ga[á?œG'놘,?§ga[á?î"x+™:?_¬'p?¦¸}FoŒZ?_¬'u?í­³^lŒ?§Öl€./E?²'e›Ÿc?§Öl€./E3FGL J1659.7-3132@vØ¿p@¾$çùÀ9;\WìÀ:úszK ?ØY¬Þ^´@
<În7–@7ˆàcØm¿ãV<=%­í¿éÙÿÒL'S¿Ôš©ùQÿÁ¿ëR@¶˜GAGNbcuNVSS J165949-313047?íN°Ãuzs?ºžSaž£	?µŠyäT,c?ºžSaž£	?í·''&?¼¹Ók›É?²FÆÆÏg<?¼¹Ók›É?èѹîãtq?³†Kƒx?̹Dr.7?³†Kƒy?ëJþî€?··m"<¦?ÂÔ¼G­þ?··m"<¦3FGL J1700.1+6829@X⪀J@Aš¸GÀ7õKÏknÀ;2ƒ
?ñs¯g6@šÿ¬óéq@/EnÛ*¿ãúpø]¢¿åÓFœz'A¿æ`¢›æ¿ê2.™AGNfsrqTXS 1700+685?ï÷ó'ÚFn?I³Š*Cõ÷?PÚKs!l?I³Š*Cö?ïÓî·?'1ãVþô¥?vô¤z€>?'1ãVþô¡?îʬeà?—š¨.CL?£U?©¡þâ?—š¨.CM?ïþþ§¤ñ? Ø"€Lì? …¾Pó{? Ø"€M:3FGL J1701.2-3006@v{ 1ί@=ñÀL5äÀ8™'è|U¼À;§ú…l¼?üê·
ÈÀy@ÉþºÛˆ§?øDÓò0±¿Ô'\лnÖ¿àÕë/³L¿åÁáìï'¿éœ!3OTHERglcM62?rü=Åþ?qmHï4H?ïÛÖó"t?qmHï4H?%êže=?°nŠ¸Ýø?ïÎЫÖ?°nŠ¸Ýø?´ûÙT4¼?¯³'ÙÃfþ?í`"Þ5yh?¯³'ÙÃfý?ŒeFánql?u¾3G‡ê'?ïŽjäzF:?u¾3G‡ê'3FGL J1702.6+3116@J³Ÿÿå(
@Aá.ßç[ÄÀ:T'Íó=zÀ;Øèd?ð¼48Á½z@Ó/ Tk?öV‡¡ž&¿ëRHíã%‡?ïøvP`·ó?¿ØSË{‹^?·%ÂåËÔÞAGNbllRX J1702.6+3115?ïÙéŸEŠB?w€Ô¢Õ?s0]:ß?w€Ô¢Õ?ïšè‹W?˜™dû½æ?‰Eü*8æ?˜™dû½å?ì•Ì-jú?¨/îCèe9?»Q›†"¨!?¨/îCèe9?îьÿ®18?¢Â_Zԉ]?¢ç0ì‡?¢Â_Zԉ]3FGL J1703.6-6211@t'%¶™…À(Ü>úç'À7ðª4À;?úVôÙ?ìÔ:>a±î@…g;Mˆõ@È£Ìhú¿åE:‡:qk¿æU/ø¾¿å²Ê]ZÚ¿ìÒºû15AGNfsrqMRC 1659-621?ïÛø	¶ e?lÇܵ%¯z?rû$¯Í<?lÇܵ%¯?ï¼'ŽÙ?‰ÔUYՂ#?€üöI½*?‰ÔUYՂ#?îD[~§"? ‰Ñ,vGÐ?«ºO†»? ‰Ñ,vGÏ?ïø/µ²§?KŽ÷‡ù×o?OA)7í`¨?KŽ÷‡ù×{3FGL J1704.0+7646@[;ɟâÚ@@3S 8"¬À:gCÛ÷ãÀ<´SYCh¿ÙúhöRq@"cW=@—$ žE¦¿æedÿð ö¿çaÕN•S(¿æõ47?1n¿ïþëWýBAGNbcuNVSS J170357+764611?ïÿ}K°ã?+ÀGÏè?V‰íã—0?+ÀGÏ?ïγÅðÅ?OTçiÈv?xø&ž"?OTçiÈx?ï̱«ŒŸc?zd¯:TC?y§*9°NŽ?zd¯:T:?ïópÎ[Z?TG[àÓ0?YcIéKW?TG[àÓ=3FGL J1705.5+7134@Y¿B¿˜0ä@@õ®Ú«³À:¶ïº€À< VrÓ\3¿÷ýò ï8Ý@ùÛQÊÍï@'¿_Ñ̼¿ç[¸b‡‰¢¿éeÈ­´¿¶x,rµæ=¿ïÿ"m¾RAGNbllGB6 J1704+7138?îb.®LÁ?·Gb×·õÝ?©ÝÅ3û?·Gb×·õÝ?ïoè Mø ? ,‰ùýBI?'ûö@ü ? ,‰ùýBI?ìZçæÓ ?µùí§+Ûá?½(Àρc?µùí§+Ûá?ï÷ó"*ˆ?Y"õO`[?P׫þñ²?Y"õO`k3FGL J1709.6+4318@QŸÞW9@BƒÀ€æÀ7ÇÎÄô'7À;7[‹AB?ö(ƒFÆãÕ@b!LÖÈ@Z"tf"¿àóÛõ3É0¿ä³"›Çµû¿äÛÖS‰?¿éU*m¬AGNfsrqB3 1708+433?ïówà-?U	WX<À¬?Yà?¤Åç?U	WX<À±?ïÖmö汕?€^¸™?tÉŒ§5š?€^¸˜?î†1Ó{Ba?žé[{w™6?§œâÈKÙó?žé[{w™3?ïÿÞ¸"§d>÷ã(`¦gL>ð£î¬Nƒ'>÷ã(`¦g3FGL J1709.7-4429@uq"_ôöÀƒu€_¶ÊÀ4s 	ŠÃ=À9Œ";±†ö@
Êϓ%·@îô¿ÚöÜ?ô…¼/E½Ï¿Ñ3JøLt¿ß[o˜ÐW,¿äDb"4o¿ëž©<·ÁPSRPSRPSR J1709-4429?4ъ©™u?5Í4mñ{!?ïýeμŠÍ?5Í4mñ{!?'¢¦õ¹úê?DÅ­lœ)5?ïþ…Ր¤`?DÅ­lœ)4?x¬';Z:?tÊt&ZF?ïΦÝó‰L?tÊt&ZF>Ôìø9jó\>Ýg‰§áu[?ïÿõ‰ƒãI>Ýg‰§áu[3FGL J1711.5-5029@u&¸!ïÀã
é`À9W4Ïëe>À:ûy€žQ¿ì~Ì¿%@÷þ;¯®"@võ_"
Ž¿å2­[O¿¿í"š¿\æ¿å$˜ÎmG¿¾•`åHÈAGNbcuPMN J1711-5028?ïìµ	üͬ?i¥¬¡˜m?cJö2T{?i¥¬¡˜n?ï_¬ø–6?¦Áã¦Áø?"
`í?¹>?¦Áã¦Áø?í~Dº¬?¨Þ±!;ƒ?´
ßWB*¢?¨Þ±!;ƒ?ïþ«œd?$@ÜCHo?%F7îIÓi?$@ÜCH3FGL J1711.6+8846@^kYáó¥@;£Ó £ävÀ:p*ÜLœ'À;Ï(†1?âSb;+ª@
>àI+m?ù€@'&5¿î
rÓ©'?ÚtDìÍ¿ªmvûßßÏ¿ÇöÀÍK^	AGNbcu1RXS J171643.8+884414?ïßÊ6'#®?n›¢´Ä÷•?pä·n("?n›¢´Ä÷£?ï¼ÒÉ{×?‹æKŽLra?€ûKM¡	Ï?‹æKŽLr`?ïm¹)•
?ˆRÔ Ù©z?'HÚßM^P?ˆRÔ Ù©y?ïUë<2H–?±G¾*?•B˜y¶íL?±G¾-3FGL J1712.6+2932@Iýöÿ¦=í@@ ƒ?»òÀ:D,_Ú[+À;›Ýj©Â?èàðÑlwU@Öa¤J"?ù4ŸWž¢?Õ-­zË?ï÷NÈKD¿ä¯ÀU"ÏÁ?Écu‡ãÛÿAGNbllRX J1712.8+2931?îLdÊ¿ø?ª×Žr#Ýô?«9³TŽ?ª×Žr#Ýô?ïXÔZ†?¥"¦xl>?"þt¿¯?¥"¦xl??ìÒéõ_tæ?«³'‹¿?¹h°UXÆ?«³'‹¿?ìÏ£‰Û¥?²óòß0?¹'ã·™"Ó?²óòß03FGL J1713.5-3945e@uµ`ûH
¿ÞCë c¼'À7m÷¤ç«À9ڟ¹nK7?å…ø¼X¥!@
t×½ìŠ,?ùú¿˜†Ê?Ñ$†<oœñ¿åÅoá9k\¿ÐJ)"]È2¿¿þE?Ð$›OTHERSNRRX J1713.7-3946?ØL(qT•?Ï/¤Þ ç7?ãÙëÇUµ}?Ï/¤Þ ç7?ã­¼¯ˆåó?ÕùÝË?ؤ† î4?ÕùÝË?æ,þF;?µéHzõ‰æ?Ó¦s‰Óñ?µéHzõ‰æ?ëéòhwêú?¼³&æD'?ÀX6^ T?¼³&æD'3FGL J1714.0+0748@<È%ŸÌ¹'@9/(Ÿ[zzÀ9cÇÚõ"|À;hèz0H?ùÐÄÔú@
ÕÑò¦{)?ûڀ׫Íú¿äþ̍¦‹¿ÖêDEÃóN¿àfr†ýr¿îÂÖF¯MPSRPSRPSR J1713+0747?W²;äú¥'?VBö°æl8?ïô&â
'¬?VBö°æl9?ŒÇ*A-Œ•?˜&.w²Â?ïŒãVûIÎ?˜&.w²Â?®¬ÆÄãw? {7÷Z?î3"±È? {7÷Z?™Ä)šËR?Š".Яìò?ï1Þ·#)¥?Š".Яìò3FGL J1714.1-2029@	µŸ´Á@%,ê¿üÚ²À9åRÒ4ëšÀ;;h7÷¾?ÙÅ¿'6{'@{6¢0—?õ€ïÿÕÙ¿ïÿñã?ïøËùo˜?Ù8'2"t?¯ÄõµE¾óAGNbcu1RXS J171405.2-202747?ïùâzhÐ?KNz+å?d?Hv_è¼ÿ?KNz+å?^?ï̎ön]N?ˆÅNh÷:?y¸"ÈÑYŽ?ˆÅNh÷:?ï̂tMX?™)ØY®P?Ÿ&o±vU?™)ØY®Q?ïõ:Ô»1e?d½¬óµ?UŠV‰5?d½¬óµ3FGL J1714.5-3832@uÆìà2Û?³´à
ŸÀ6‡à3±ÞÀ9©Þß)?úžÉ|5Z«@ìNµo¸õ@g(ñ:ë8¿Þ]›ç|¦¿â¥¯¢šÜ¿ã¾¬B鉜¿íÕÇGQÎOTHERsnrCTB 37A?w ›½qìX?"új}÷]÷?ïоȅ'?"új}÷]÷?[[/2ŒKb?püEØÈ?ïòRhf¹Ú?püEØÈ?°Èçím¤Ï?§_虍?íæãRKf?§_虍?¡ã>Èûá?"? T'~Æ?îáÌpAð?"? T'~Ç3FGL J1715.7+6837@Xә`#VF@@äå@a À9˜hô¶âÀ;Û k°R?õeڍ)ɨ@üÓТ?ý­ËOt1€?ÃØÑgç¿åý–Pía¿å(z‹LÇ¿ã
¯ÃžóAGNfsrqS4 1716+68?ïûmkú›?MÌàáh*?BJS'Ú?MÌàáh?ï~º?ÃÜ?™jDôÐ?(®X"'?™jDôÐ?íŽ.4÷%?¦ÓŸ£cøš?·ËŽŽXFÜ?¦ÓŸ£cø™?ì÷»æ@÷?¥ù'$̧?¸Gb ÍøD?¥ù'$̦3FGL J1716.6-2812@vRÿÚ@S@ä%_µóÀ8ÃÆé]ýÀ:Íõ`iÍ#?ñMD¼rŒ@ÜJ)ÄÊu@ê@¿Ê¿â¬
µe§û¿è&Õ¢}þ¿ãÕíݾŒ˜¿ïÿò"²¢OTHERglcNGC 6316?ä"ô_ã±?лOÛîíF?Ö×ò@8ž?лOÛîíF?Þ]À×sþH?Ñîv°à¸5?àÑ"FÛ?Ñîv°à¸6?Ùl¶$tîŒ?¼H'ÌÆSÁ?ãI¤íňº?¼H'ÌÆSÁ?Ò#5Ü2ñµ?´9D*<ß ?æîeæ‡%?´9D*<ß 3FGL J1716.7-8112@s{ fèÀ7U* ½zIÀ:—íùm?À;Îú2`¥\À
ü¶!9¶…@
æÞÿ)k^@zñ –¸ê¿êÐ熿î'ß«¡¯?ès›s
"¼¿ç"!šYïAGNbcu1RXS J171712.6-811501?ïÿë1N ?$$:@Âa?™Ö<q?$$:@Â`Æ?ïïÍ}©é?kži=®M?`ð2'VW?kži=®J?ï£êf}‡³?…wò½Ñ2e?‡f`žü?…wò½Ñ2c?ïÿÿë°È²>òOïâªH>dO7N¾Sß>òOïâýÃ3FGL J1717.4-5157@u»`(^ÄÀ (g "I×À8›.­'tâÀ:îs#ä
×?íŸÃ'™þ¢@Í? §?@óNi¿áµh†•ö¿æqÃóà7¿æ6ö°RÄ¿ï1æáPãAGNfsrqPMN J1717-5155?	ªÅ>?,øâÞg?½•N°ˆ?,øâÞf?ïQiùb"?¤èPÎ@nx?•ÒÀÓ½­y?¤èPÎ@nx?ìëh@âóW?§ÒñKêÏä?¸¤½øèeJ?§ÒñKêÏæ?ïø/¥ú•Ù?Kªº€È¸?OAh¨›ë?Kªº€ÈÙ3FGL J1717.6-5802@tÊ*Ÿ{ZêÀ'¦þÜêQÀ9KHÓ®hÀ;_	Ÿ»òŠ?u 5Ø
¥@÷¥LUC(@]€†£¿ä."Š]‰¿ä <Ð.Åտ䅄 |üo¿ïü¸#Œ:ûPSRpsrPSR J1717-5800@?ìÍÿñ[»?¹M[Hhà?¹ðu".?¹M[Hhß?é®;^ï?Ê­S¼öñ?ÉG‡³"C?Ê­S¼öñ?è|šOj?³ƒ¹j2`>?ε–ÂWÐ?³ƒ¹j2`>?ìø@§¦÷•?ªŽÛв5ÿ?¸=úÂÈCN?ªŽÛв5þ3FGL J1717.8-3342@v/€Uûµ@ވj1À7,ò³"À:(zúr!†?ðäH™w@ðU+%É@HkÀmmí¿å—Ì<%—Œ¿é3‹fŒ¿å¢`°ì¿ê½]¡¤^AGNbllTXS 1714-336?îr@;ú¡Ë?«ÚQŒÓt)?¨Ûü@Uã\?«ÚQŒÓt)?îǝ"Ý>¿?¹é|¡Ä?£†-Ò,?¹é|¡Ä?çïY<¾Y¥?³Q*¢Š@?Ð!M†ƒL·?³Q*¢Š@?ïÓ8"d)?sêÚ÷Àߪ?vcµÍõëÅ?sêÚ÷Àߪ3FGL J1718.0-3726@u۔€u?IJ¦ ÷­‡À7¾"Xð\À:I窞¥?Æá-;¼@
Òfhe@+äU¿çß'¶ÿ¿ãáäŒ3 ¿ß"ÂÇæ¿âœúÂSw OTHERsnrSNR G349.7+00.2?â·¬`Pˆ£?ÍhÄâgkÆ?ڐ§?^î¹?ÍhÄâgkÆ?Ý<3ƒšŒV?Õª1˜l‰é?áaæ>2¹Õ?Õª1˜l‰é?åƒÌûáoï?·¸¯o‡?Ôøf= #?·¸¯o‡?êà¬üh?À}ÒcuŠ7?Åø}Oˆ^?À}ÒcuŠ73FGL J1718.1-3056@v0÷Ÿ©~@ !€ƒHÀ8É&رÝ]À:»_"K|?ä™fîC@ÂN™–@þŸßXë¿Ûi;9ßA;¿ëV¹"uÝ¿å#m\=²¿áTn‰ËpVAGNbcuPMN J1718-3056?çŒÛϚÁ?Ì5]‹?žˆ?ÐæIâ`Ê?Ì5]‹?žˆ?íðÉÎÕs?Á¹I!š@W?·8y±‰Tb?Á¹I!š@W?ã(lf<?¿­}ˆä?Ù¯ãÇ'3ˆ?¿­}ˆä?æ5aõKQf?ºñË{Ü$Ô?ӕ<i]4?ºñË{Ü$Ô3FGL J1718.1-3825@uÏÀ7"¿Ûe}`††À78CæߝŠÀ9¿6n@O@!w¤QX@î!è2-û?ÿ£NÏ?æl>;ÇMÔ¿âKW€–¿æ»\s¸"`¿ïIV^0ÎPSRPSRPSR J1718-3825?t?Œ«eÛ
?†ÞN'™?ï׀æ©4J?†ÞN'˜?D=¿-Ýþ?]<x。?ïúð¸P4ˆ?]<x。? .àR?¡9/[ÃÿÉ?îÿî
Aû?¡9/[ÃÿÉ?æRf?wn˜Òà½?ï¹û°f¶g?wn˜Òà¾3FGL J1719.2+1744@CÂIàâi@<A_EàµÀ8Ãp@Ú»£À;L':ƒŽ¿è*"öØ[@³>\;-@WhÿóÀ­¿à;Ý
·£›¿à%–¯Yl¿àÿ[Ikž¿ÛÆ;IheAGNbllPKS 1717+177?ïÿ"?ÿæƒ?òN"ðM?¸/§?òN"ðLŸ?ïÞ§ŒÆqÙ?|d6Ï¿?p¬9œÇ"?|d6Ï¿ ?ïʉ6q›Ë?z.¨öŠ¸®?z»dÇ2"?z.¨öŠ¸¥?ïÿÿ)I<>¤fp§>Ý=>žzÖؑþ)>¤fp§>¾3FGL J1719.3+1206@@ÜLŸëÃ2@9Ö4 ˜ü¼À9ð5³@3ÍÀ;~#yÌ?ÞüRF…@Q8!.£×@ŸŸ÷ג¿×r¯'¨ï¿åêà`ÓT{¿ÑŸ!='\¹¿Ø]0Ú_ÔÉAGNbcu1RXS J171921.2+120711?ïÓ‡éŠK?~u,Æ;ì?v|¼:ÚI?~u,Æ;ï?ï5ufä!Z?¢.ÇüžlÝ?™QS#{Ôä?¢.ÇüžlÝ?ï.v^æ‰?'é ¤šmÒ?š14#<.Æ?'é ¤šmÏ?ìRÂ)Yã?¯ºÉ3D¥?½iî·Ý0á?¯ºÉ3D¥3FGL J1722.7+6104@VŠÆŸ÷¬@AàP7PÀ9ó¡gÄ4xÀ;ŸáÝÖ
?ߑ±ÿÓ«@{7*ŽŸ@øýŸÓo~¿è‹t­¸¿êTÓSFŽ¿ë¤3Š\]¿ïþ™øRü@AGNfsrqGB6 J1722+6105?ïõ¬!"L<?VzðÐï_?T§½»g†m?VzðÐï_|?í¨º^k3ç?´‡$(ë?²º-¦`Í?´‡$(ë?ïNã¦
Ý?'ÿ݁r?–#‹>D]u?'ÿ݁w?çS tr¸?·©~ö5¦?ÑX¿ð'?·©~ö5¦3FGL J1722.7+1014@@m ‹]@8M@LzÀ8ˆéR>'5À;86%UúÞ¿æä¨Y·¶@˗I]A$@`Ÿ l1,¿ßýZ¸w+¿çÃÂÔj>Ò¿àqaûƒÕž¿áÓðÇË'©AGNfsrqTXS 1720+102?ïÿÉe禭>óã‰Z=X>ûM,©4?>óã‰Z=U?ïٻٳ?~,˜Î¼2?sq¢&€‰?~,˜Î¼5?ïÊZ£Õ¢¬?{
m£Q?zÒ®.ª)?{
m£Q?ïÿ\»£Â?vKÿöI?h‹ÇÍ
?vKÿöl3FGL J1722.9-4529@uz!@W%À«"ÿٔ†À9ÍSÛIÀ:°;C¢ìÿ?ԋŽ®Ùò¥@
­ñœÆ@ÁeÖt¿ã@4}áb¿éÏ"¢¿³¿ÙwÜÛb½¿ïÿîbHÊtOTHERspp?éó†e3f‰?ʚ÷Þóo?È1æk2eÛ?ʚ÷Þón?ä÷EîCô ?ÒO'üWç?Öt#xÁ?ÒO'üWç?æwٛ,B?´ÕB».?ÓLɧÙ}?´ÕB».?é
Üã¯-w?Á.3å",?ËȌqCJ#?Á.3å",3FGL J1723.5-5609@të¿çáüÀ&IFÿ˜ÑóÀ9ç**¾ðÀ;VB7²ô´?°_홃Ç@Lêik@ñ ÀTnl¿èæ¯æfÿ¿êò­Ï†}¿Î}$ƒmj¿ç×a"¯­WAGNbcuPMN J1723-5614?ïþy…›´?4£™Íj©?(g¦D¿¨1?4£™ÍjÆ?ï'ÐxæKý?˜§æ9Ç)?KáÆmû?˜§æ9Ç*?ï™vÉè4?†ÒÚl?‰¢M…û²Î?†ÒÚn?ï˱ţŸ`?s'ŒÏ½³?z'.0P??s'ŒÏ½²3FGL J1723.7-7713@s»	 'RTÀ5˒€ ¤PÀ8ê̵O؅À;nÐ6䘛?í¢ز¼´@O·3ÞSÞ@ü?¶Ï5¿åQ¶†íοâù)Î'¿éØ8Уhr¿êú¹…$öAGNbcuPKS 1716-771?îø©œ?¦ž1Š{]ë?¦ÿuf@?¦ž1Š{]ê?ïÄ琞ð?…†§©á?}õŒ7°‡©?…†§©á
?ëSï%L×?¬˜Lå zX?°CjÌ¢?¬˜Lå zX?ïn´™`,?ê6&ü?ž')lÓú ?ê6&û3FGL J1723.9+4004@P8Z€¶–@@–ôÿñ½GÀ8ÕÁw.4ÇÀ;¨"Æ£½à?ó0ºø¹å"@¥³ŸTD@œÏÀr "¿äs°¢"¿å›{4îc¿çÂá_'
¿ïÿÇ/ß_AGNfsrqS4 1722+40?ïò¨G¥uä?Z%]u{}?Z¯pµ5À?Z%]u{Š?ï´3ól®?‡ª­Îö\·?'óÃ$ÔË?‡ª­Îö\¸?í2–ñF?¤Š+®¨?¶o{HwíÊ?¤Š+®ª?ïQ
L7•K?ˆ¼°òˆMR?•Þ¶y
V¹?ˆ¼°òˆMS3FGL J1725.0+1152@A£_ëøâ@8|H 'ÁçÀ7ì=s(À:½ ùt˄?îJh[´×@…¬àa?þ*?›Ü?¿æë'Éý¿ÞÓÔmÕñd¿Õîqsp÷¿×e:´SP¬AGNbll1H 1720+117?ïøMò×e†?Q¬EÆÓ?NÈ4¢iç?Q¬EÆÈ?Jôև?'ꎔ)ϓ?‹­BÊ^ƒ?'ꎔ)ϒ?îÖ6£#äø?™h¨X³?¢œ•ÍÁ°{?™h¨X³?í=bý‡Tp?£ã"3ý"?¶èÅ\|?£ã"3ý"3FGL J1725.1-2832@v^"@lÚ@û6à÷IÀ8·N?(3üÀ:†–UAzõ?ó³'6{@;e[Ï_@Ìõ U p¿äÀ€æDm¿î¿'Þt†¿Ø+¸ëny¿¼Ç5oùbOTHERspp?îgxÝgíí?¯d ¥W?©ˆr)!.?¯d ¥W?ïs
k8?·ç$uN?'ž²˜ý›?·ç$uN?èš77Ѹ9?°ìpƒ³hB?͗# ¹?°ìpƒ³hB?îQì­F?¨¨¾!®E?ªá5+žé?¨¨¾!®F3FGL J1725.3+5853@Ußϟåãõ@@ÿŠßÂr×À:cµ±þÀ;ïLñJZ—¿éù@ö#Ÿ†)@no?þȝ¿á ÁCà28¿à«¥Îö¿ä/vve¿ãñÍhAGNbll7C 1724+5854?ïööc??f´¿Ó?RÙ9Îl?f´¿Ó?ïÐ
Ž—të?€I O+Úî?wú¸´E‰É?€I O+Úï?(÷Jƒ?ŠØx''·U?ŒuÂ-_"?ŠØx''·T?ïúQ­Ñ?CÏAò½õ?Gê¹H»éž?CÏAò½á3FGL J1727.1+4531@Q܇ Q»@@©÷¿¿žÀ8¢Ëlz|žÀ;¯ß´tç?õ`]æe$G@{bcL@¡\3\£Å¿äZÇ´Š
Û¿æƒÿíFâ¿émKŽ¿ïÿ{z
§AGNfsrqS4 1726+45?ï÷€Á)áç?Q*ä§ò?Pþ}¬<5´?Q*ä§ò?ï\-H«?™ã~¯x?"z]¿öê²?™ã~¯x?î˜ `Í¢?™‹):Ë?¦}ùó%ߘ?™‹):Ë?î	h¥›Œ;?¡ðšüþ%Ä?¯iu¦G<;?¡ðšüþ%Ã3FGL J1728.0-4606@uy¬¿±[WÀ
€F6pÀ9:¬.Ǔ¨À:üº·÷R²?ÖQœˆj@
×i0EB)@x?V×þ¿éÀ	oëJ¿ß<Zú!™®¿àeýö:"`¿ìÁ°~ã_áOTHERspp?Ànãäðjš?Â1ùTÄÖu?ëäGÃåY?Â1ùTÄÖv?ã¯m¬éµ?т¹C*W'?Ø¡$¦-Ԗ?т¹C*W'?ÞQA&VF?¿clŒáPø?àþ×_lÔÝ?¿clŒáP÷?çõK.úL~?¹ßx=:?Ði¢g?¹ßx=:3FGL J1728.0+1217@Anž i—s@7þγ#®À9u;â.]áÀ;= 8Ûê¿å´ñÙ÷'®@ï¼C͈@@w˜¿ÓNŸ~ú ´¿æ¬Ó;ë'^¿ã¦®Å¿é ›Žf_°AGNfsrqPKS 1725+123?ïþ(%
ýQ?4qËgË?-}¯ *ße?4qËgË?ïӓóØ)?€˜Îá=äu?v6v"ëí?€˜Îá=äv?î¾ÒdÀH?š°É#:4&?¤ß9³û€?š°É#:4'?ïùž9nW?DÐú‹]²?I‡GÞ«5?DÐú‹]¿3FGL J1728.3+5013@SE@€"Ð@@ÃF߸aÜÀ9!EºtÀ;~JÏ1+¿ü=¯
@ìuN‹©A?ÿ[–~²­¿áÛ0–†ûÿâ*"Ô€Þ¿ÖmæÚ·i¿â$í|ÓAGNbllI Zw 187?ïü<ý-?7ÏÁy?>ޗy?7ÏÁž?ïÐÉwBùÔ?€¾l$s?w›D^ƒ'?€¾l$q?ï«6͊"?ƒj)›þq?…2xLwg?ƒj)›þu?ïÿêõC?)5]ûð}?¡\—"˜?)5]ûðà3FGL J1728.5+0428@;W¿PãG@4sÔ Ö¤½À8îdüÀ;Cí\M?òˆB+ž"U@Ɉ$Ì@ÀÿÿÕâ¿ä«ZÌ ÌÌ¿çÒ{•w ö¿é"i+üÄ¿ïúÊ;ÅJAGNfsrqPKS 1725+044?ïå#¦Ú,¶?re#INµ?jÜY%ÓHÅ?re#INµ?è¹|gu?ƍ=Ǩðø?Íc«Â,?ƍ=Ǩðø?íba‹ßê?¥µÚ¾•›?´ìó¡¯î?¥µÚ¾•?Ø2åJ¯%‰?±vT
N™é?ãæZ¨m;?±vT
N™é3FGL J1729.5-2824@vhË@p2˜@
!ç@–sÀ8ÛwˆÍ™{À:¬¦]¨R?üó…†QŒ@^köÝ@RtÈ©Òw¿ÊÃõùó¿êÄȼœÓá¿ìd1Xh¿ïþûB0&OTHERspp	?¨ËbX¶Þ?²–º·Í¾?îsIÚt'?²–º·Í¾?—½ÿI"à?°¦ñ]Ì?ïBõ¶è?°¦ñ]Ì?ÎñÒ>)S?µü½iÂY?èC‹ypu¬?µü½iÂY?'òLYp®r?…^¤Ç+?ïhm4z?…^¤Ç+3FGL J1730.5+0023@7ÄÊÿm3	@2-ß6[ÝÀ8Aðþ}=À;ÅJøK×?𭷀µG@×6aæÏØ@ƒ@7'´¿ßùnurý¿âh!š*¿âqõvlÌe¿æ'>×+KAGNfsrqPKS 1728+004?ïüõZÍa?7†OÑX²?8U)"÷Dâ?7†OÑXÂ?ï݁˜=¶´?}Ó¼Q,°–?q?3á$¦"?}Ó¼Q,°˜?îógÄÌ×_?"ÊvN/"Û? Éƒ³2Š?"ÊvN/"Ú?ïïµ?AP$?UG1Óã«?`JÀ¾¯Ü)?UG1Óã¨3FGL J1730.6+3711@Né"åx•@?\
ÿ7ƒ$À:p¨ß‡ºÀ;ÐaP?í±½k[@yò'>N@³À€8Iž?ëQႢ˜W¿å˜tÄ´5¸¿ÛIlΒþ(¿æüŋÃu¿AGNbllGB6 J1730+3714?ïñĸ|kî?bƘÑ?\v($ª?bƘÔ?îHƒìä'?ªÊïM)ì"?«wÁ?A·ø?ªÊïM)ì"?î¿W7)p?£3Dˍ?®"
Œi?£3Dˍ?éhyG°ØÎ?±xUª˜a?Ê^á<œÌ?±xUª˜a3FGL J1731.8-3001@vW¼ ?ÿC^¿S À8~ŽŠqÞjÀ:…‡ú4ää?ðD%'_
'@
®>lL?ÿÅ*A*¿åf?²ûóß¿ÊKf»uâZ¿âD˜L׿á6g\IpÑAGNbllNVSS J173146-300309?ê¢X7ßP?¶/;&˜ü?Ç©vŸ 'À?¶/;&˜ü?ádÕñB$?ґ§œò?Ý7þT{¹?ґ§œò?æ0$à?·³Í=ÃZ?ӟϷõÎ@?·³Í=ÃZ?⯼/?¹K?¼Ðíó2È6?Ú ‡¡€j?¼Ðíó2È63FGL J1732.5-3130@vDüÀz®ó?ð?8?®ŠÀ6 ?û˜'3À:3X–š@
u9ó–»@FÿÙ> $?ëÊS0‡9ù?ïÿ(#,!¿ÂwÕRò.¿äƒÊ'´'‡¿î3&‹ÉPSRPSRLAT PSR J1732-3131?·Ë#Aø?ɹûÙ ¼Ë?훝7Àþ?ɹûÙ ¼Ë?4}I
?bÉèzö´¿?ïýp\VÞ½?bÉèzö´¾?À=2°

€?²†"ª²¦C?ëð³Sý}^?²†"ª²¦D?ñ¬"çy?iidÄ?ïÿr›g@?iidÄ3FGL J1732.5-5048@u@i³únÀ"ÖÃà'TÀ9}:í;ØÀ;W
V›H?ÔÂS*ä@$QËú"Ü@Fk€V§'¿è¹?H·¡¿Ýqtºf³¿èú4È«ø¿ìê×ýêPSRPSRPSR J1732-5049?ⶣÂeÁÀ?Ë}éáÆÍ9?ڒ¸{4|?Ë}éáÆÍ9?í²c:Í4¬?¹ª¸*jJ?²læ)–Z"?¹ª¸*jK?ç!owhÉ?·Zt?ÑÙ½!.n?·Zt?컶L":Ä?£–µæ›ÿ´?º"M›Þ)â?£–µæ›ÿµ3FGL J1733.0-1305@(÷ÞÉN"@% 6^`ÞgÀ7'ÎuCxüÀ:¸M`Ûâê?õ5ÁB€D@Ç2]Ë7K@éð»>"ö¿ân¿«œë¿æ'Åeòš‰¿ä­cÐß׿è*»¾—ˆAGNFSRQPKS 1730-13?ïòŒÍ·?Z×q·"&?ZàædÁ˜?Z×q·"%ö?ïÏÚ?ƒÇ'V"&É?x@wwð"U?ƒÇ'V"&È?îŒúááva?žTl<V7?§0Qáè™í?žTl<V7?ïÿNø#ù?T¨‹Ö|? ì[€«Ú?T¨‹Öo3FGL J1734.3+3858@P"ÿÖåU@?…_Oñ°À8GuÇ,yÜÀ;m>m#
?ï6¨ê¼@]®:æ[@€…Zmà¿áj0]Égp¿å­è…ù¡¿ãÁ5,»''¿ë_š‰ŽAGNfsrqB2 1732+38A?ïôù¨[—?V¼Ò䩨?V¯HÔ ?V¼Ò䩬?ïÐñ:Б?áu;+ä?w‡b—·~Ë?áu;+â?î1")òûk?Ÿ5ó&S–s?¬æ½`ÐII?Ÿ5ó&S–r?ïþÜí¦þç? Yåßc1?"1%¨? Yåßb3FGL J1735.4-1118@+Æ!à$˜f@&sA¿½ð'À9OsGö8×À;4žm>¿êšŽÇ-¦@ç\20@@O¿Û͜¿Ððs{ÞÙÑ¿ëºeð°èҿΤf/0¿ØøáÎ;·¼AGNbcuPMN J1735-1117?ï÷¢"ŒÁz?R³'ävéP?PºÖæ}F?R³'ävé??ïä E-þ?~»:EŸd?kôߺÒ‡?~»:EŸa?î®0Au_?X^ÑïÐ?¥ûï8ª?X^ÑïÒ?ïý·ŽzZ?6«:—Þ½?7:CŒ-#(?6«:—ށ3FGL J1736.0+2033@F@L j@9k>¿XpÀ9rêUrùÀ;P…Ûv³¼?ð%ä‹Zf©@sòoɑ"?ûŒ@ Y&b?ïþI™HˆQ?à6¦,Wª¿Ø^~ŽXüN¿×–fUÁÊÞAGNbcuNVSS J173605+203301?ïíèߪ?fB^ñxÿ?bâô Uí?fB^ñxÿ?ݨƒB?"i—ߎ> ?‰ȕß/}?"i—ߎ> ?îöîÅ? Ü÷…'Ÿ?¯žcŬ? Ü÷…'¡?í¬²?[Æ?¥ôŸԒ^?²šk†!Ö?¥ôŸԒ]3FGL J1736.2-4444@u˜¨ÙºÀïLßזÀ8ZHùn‡À;S‹'?ó1£™D_@ˑô^·@'`gÁ¿å±öy|Ä¿àÀЪ§Þ׿æMÞzt:d¿ï#û½{ 2OTHERglcNGC 6388?[[Sœ—ó¼?aµ*Œ¥M?ïòRV1´?aµ*Œ¥M?}e(£?˜6uúˆV?ïÅ5óÏǯ?˜6uúˆV?¸cSÿ2ï?¥ÝŒUÐ
?ì󟵀¢?¥ÝŒUÐ
Ž?°Ô%9h?œÊSº9	?íå{N^˜Ó?œÊSº9	3FGL J1736.4+0634@>EÑ q$0@3¤:?–îÄÀ9 QJuoÀ;G›	b@?í10âKF@êßp"eù@فà?pX¿è'%xyR@¿é
ÎM$¿è@doÒ\¿ïþ÷‰[U^AGNfsrqMG1 J173624+0632?ïý.ï*°¿?8¼}JÜû?6ˆ†ªz¡?8¼}Jܾ?îÍÁfÄ@S?¥þ(X¢á€?£#铻úá?¥þ(X¢á€?ïýlvöG?'Jâ'?œ@Rq!7%?'Jâ'?è\HÝÙa?­ô^F¯Ýr?Ύ߬ˆš~?­ô^F¯Ýs3FGL J1737.3-3214c@vD*Ÿ{Zê¿Ï*À1äÀ8kógkI$À:|Oø?óÁwO>'@'ˆíNø@$H¿aL¿È4ì›Ê u¿è6U'Ìc¿áȵ¥8¿æÕožŒÙOTHERspp$?²
9¼)ãý?µîê!SŠ^?í¾XÈzÁ?µîê!SŠ^?ԁ*`öd?ѽƒì¯C?å¿jÏû"Ï?ѽƒì¯C?×èn
mt?ºW‰zz£]?äȱzÉF?ºW‰zz£]?߸,þ"¢Þ?Âz'ÁIÿ_?à#é€î®'?Âz'ÁIÿ_3FGL J1739.0+8716@^Þ˜¯@;ñ¢@1HwÀ9§~b®–À;Ýî­È$Ç¿óÅΞ^$y@r6xâêÆ@7ø¿Äс¿ÔcÏÁ&"¿çÕ¬A3sl¿Ü
û˜/ë¿åŽ¨ê¢ÿAGNbcuNVSS J173722+871744?ïÿÒƬ)>üÓ·œ¢>öœ©¸k‡
>üÓ·G?ïÝ~Šø)?|CŽÙ­>?qp@ºƒëf?|CŽÙ­>?ï°f'¤?ƒp\Dkv?ƒævVú:?ƒp\Dkq?ïÿþÅí>«Ç"pW¹>£¨ñ-{å>«Ç"po3FGL J1739.4+4955@S8ß¿î—ù@?¹´VÝ\À8à±é·ìÀ;¨Üôb=¿½EÄh@9¿ím@tÔÿ÷«¿ã68š6ˆ¹¿ãG×æÂ}z¿èÈ¿%璘¿Û¢'ĹAGNfsrqS4 1738+49?ïû¥­FC?Ggi\êèÏ?AiJæóÞ?Ggi\êèÅ?ïÔh-«˜?€Óã"ܾ?uËé*3øÂ?€Óã"ܾ?ïY›!}?‹òvF"–?"Ì›Ð]<<?‹òvF"—?ïÿå‰9Þ>ï:ª®ò>êvÆb!Áà>ï:ª´Æ3FGL J1740.3+5211@Sム3Ï@?Ê.Íû¡À8|6™AÀ;¢¡€è?íú9wEï@Úæ1ø @ž¿\V˜¿â@þŽ`¿ç%ÇçØ
j¿é¥Oê<ãû¿ßÃì]$¸
AGNfsrq4C +51.37?ïúÑѵ;?DÓjü,l?D»À¹+&?DÓjü,r?ïÒ³A¶4V?'¨*¯?v¦_$åÔn?'¨*¯?ï5ϐ˜†Z?Pù¶¨WÜ?™F
ìï4¼?Pù¶¨WÛ?ïþ¹ÈÔ6?#%·[S?$cr¾Ì™²?#%·[Se3FGL J1740.3+4736@RÀ'¢Ü@?SÂÀ®À:gø[ÆÐ4À;ìP->ýl¿ðÑÝgú*@攸‰Hé?ÿ&Šþøï?çâQ]¸q¿Ù£»vc3¬¿ÛúS0‡9ù¿ßþ«íŸðAGNfsrqS4 1738+47?ïø<'),?Z"Šn°Œ?M‹c[R?Z"Šn°™?ï؞ø¡Ú?|™NÍ&¦C?s°ô¯e?|™NÍ&¦D?ïqš
o¼?Œˆ[íEï?'̾²hl?Œˆ[íEï?ïý4*ŒÍ?6¶‹/ÝÉè?6^¯+™•à?6¶‹/ÝÊ3FGL J1740.4+5347@T[O?Ù3ã@?ã$H¸À:h\ïÅYÀ;÷Ÿ<pÊ¿ç¾W¢:@
ƍ³\cX@&"_ ¤{¿ì¶ø–‡™¿ÝKH·Ì,¿Ðú&2ë.¿àÎ[‹Ó§AGNbcuNVSS J174036+534623?ïüÖ5~c?<\Ç˹Í?9NT4êo?<\Ç˹´?ï΁۠9?mÏBžì?x¿/ãz?mÏBžì
?ï¬;¤¬ö?Pp!?‰c?"ñVÔˆ?Pp!?‰h?ï÷XJÈ8?LdWÓIO­?PáOjo?LdWÓIO£3FGL J1741.1-3053@v]:à;>š¿ÊUNÀFExÀ7â¸ø²<À:Ò³–šâ@Kڞòt@ý¸§ü´?ôdÐvû_?ä-v€dê:¿ÝW¯¿JÙ¿å–œ>‡È¿ît>ág8žOTHERsnrMSH 17-39?p­L"Ǝ?‰ôÀIäŒ?ïÞ¥Õgºs?‰ôÀIä‹?eN'å± ¢?š"q:?ïê±nN`?š"q:?­gZ'¦?¬C;³´5ª?î)Š]…Ÿ!?¬C;³´5«?§`A?|9¤ˆ),?înÙûð?|9¤ˆ)-3FGL J1741.5+1351@Bð¾@Bo@5¢Àu¦uÀ9äêÅX/À;'H¸?ñÁ˜H¶¨@"—G…@Í,@zÄl?êÕû]·t¿Ü6]`¤0¿æþ5¹['¿ê
.Ž€-YPSRPSRPSR J1741+1351?ˈðè¬ú!?Ìãiì¶?éÃÅÔÁx?Ìãiì¶?ç-‹²1í¯?ÍR<b×ÉZ?Ѥ蛜$¡?ÍR<b×ÉZ?Ô!­ø¯Þ?À7Qo–B™?åï7©¨?À7Qo–B™?Ô­`¶Þó?¼lÃ$›?å©O¤†8?¼lÃ$›3FGL J1741.9-2539@ÚÜ QÚ@XÀŸ—à\À8µlC9À:m}F|¼¿¥²ŽÙ³KX@
ש`Œß@¥@¿ ?é>ˆÅ{¿à0àÍàž¿çÖësd¿Õ¸ÁÀ»AGNbcuNVSS J174154-253743?ÝJ‡Ò QP?ÏÌAÊÿåô?áZ¼ï×X?ÏÌAÊÿåô?îXÄtI?¾¹y­[ܵ?®ºs¿H»…?¾¹y­[ܵ?æ¨Ø@8Ýâ?¶µf´ë?Ò®OŽD<?¶µf´ë?î›þ†ï#ß?£I†%\»?¦@'
Â?£I†%\»3FGL J1741.9-2054@¨u€4ì@˜ F†øÀ6Û¸KgÝÀ:˜ùN59@	ÈWQölÙ@°5<wÕ?ü&µü¦¯,¿Ñ½Zý/HË¿ã:*k¹b¿í2äÝÿhð¿ïwÅiÆPSRPSRLAT PSR J1741-2054?r7"µË?¡ÅOYE?ïۑö×þ"?¡ÅOYE?P15þFÀf?Z-Cdú¢š?ï÷çeܞ?Z-Cdú¢›?´ï¨Ç[È?Ž $I?ï‰,A\â'?Ž $D>혼~®>ìåÔ%fÚÅ?ïÿâg€Cç>ìåÔ%fÚÅ3FGL J1742.2+5947@V àè@?Ï¡àø0À9õ@UZ¥hÀ;ë½¼Ž'(¿Ç®ö£
@ÕáWHfK@hÆÿ®K'¿êН<¿ämtkH¾¿Ütû'毿áZ3RÆTAGNbllRGB J1742+597?ïÿ­sInâ?"ô"üxe?£-¤G_}?"ô"üxè?ïÒõED÷ª?ÝÍ1̽?v…]]"+à?ÝÍ1̾?ï̐—ŸÖ ?ƒ:GÅQê©?y·´0ðd?ƒ:GÅQê¥?ïñfl2<?T W7€Œ?]Û3'›…Á?T W7€'3FGL J1743.9+1934@EêG@0q¸@7Wà0VàÀ9ŽÊƒ*ÂÀ;Z´Î©Eß?ÜýÐö…¶@
(w¹õڍ?ünJ 	µ¶¿à'󆹱׿ÐláÈ¿]¿ÍíÖèY›'¿á"'¶®"AGNbllS3 1741+19?ï½Öõ'?€(×ӝ >?€¼:ŠB›•?€(×ӝ >?ï]\äڅž?—õh›¹?"Tcd¯L8?—õh›¹?îÓ+ýšš?—dÙLÄî?¢Í@&öVn?—dÙLÄñ?í°µ~÷å×?¢#¨µŒ4À?²zT@ÑE?¢#¨µŒ4À3FGL J1744.3-0353@5"?·¥ô@*
N wmÀ9œ}¬ðÀ;ŸÑß[¿Éw"\‡{›@
>µÿUá@'WÀ0\>?å#Û´ÇŠ¿åcÊøÒæ¿â݇®úBÁ¿æJ~É0õAGNfsrqPKS 1741-03?ï›ÒöVŒt?'þۗÔ?‰Bj\ã-?'þۗÕ?ïŽm
€!?—.dߗJ?Œd¼Ÿ÷ºd?—.dߗJ?í…õüH?¨¯çT7g?·;ÐP¿á?¨¯çT7g?îœÈvê? ÕÓˆé²?¦3xž1^"? ÕÓˆé²3FGL J1744.5-1133@-¦C?ñC@"^C ÚxÀ7ö›ÅÃÄÀ:Ùxà¼mÚ@.Ħ7¸@Øâ'q	@'¨ëF4˜¿ÙÉñÛÏôõ¿àÚz5Œe¿ê£Ö0Ωò¿ìÀ"•W¿PSRPSRPSR J1744-1134?I.ATÝ?AE¼I¬á?ïùœ4ï«?AE¼I¬á?gc£榩?qòÒííH?ïèœ\þX?qòÒííH?"V§Ÿ`î?HÅUøµú?ﮥa'}‰?HÅUøµó?US÷×èm?G¸¿j¤å?ïõwÖ?G¸¿j¤å3FGL J1744.9-1725@#×Àâ¯@^á¿Î¼À8Å]Ó6À:ä9]ßË¿³»ëñ-¾Ð@9òj@›Ä?àj¹¿éùrû¨µõ¿á
ąšM
¿âÛ¼…¿×yµAڄµAGNbcu1RXS J174459.5-172640?ïæÄÎ6?lt/O'JO?iâ;1Éå‰?lt/O'JR?ï¶8«ôz?æ¯P@ß?'z±Õá§?æ¯P@à?î¿Éu€œ¦?™~{¿Î:<?¤h§ö5¡?™~{¿Î:<?ï':f·'/?ƒ*Gî›C%?‹qfR´1?ƒ*Gî›C&3FGL J1745.1-3011@vmú WŽ\¿â…'€ã"À73	~.IÀ9ºrW5q@æ|®§GØ@[Yèÿˆ?üÂHÊt,ù¿âáê ó*/¿ã"±_ÞâÏ¿í@øM"Q¿åȀl¡êOTHERspp?¬y?L–'?ÄaîmÔX?î>øl6—?ÄaîmÔX?r¹Oó½y°? ''ۛzÏ?ïڍ`…? ''ۛzÏ?ÊÂØôԔª?¸=æ?Ã?éOIÂÊÚÕ?¸=æ?Ã?"µZ¸äL?''ñ\N?ï­+º•o?''ñ\N3FGL J1745.4-0754@2%ƒÀ€æ@%¦<OšÀ9ÿ}úâÀ;׎Ǯ€¿éòzv=Éå@õwæÁk?þ±Ø³iy¿é¢Å¿^ǃ¿Òïò¥¾.é¿×B5Ñëg¿át¨üì'ÓAGNbllTXS 1742-078?ïò9C$ ?U:–Šl^%?[y·¿Üê?U:–Šl^&?ïԋuývÜ?·	¨CL?uºED'×?·	¨CM?ï3P•Ú?"\TpCa?™ŽUíD¾}?"\TpC^?ï효ð‡£?dU]‹Ý}?beWx\Q?dU]‹Ýz3FGL J1745.5+1017@Alú€d>n@3BࡕçÀ9F–µ¹‹À;=4Ä,ë?øtþÂhDã@'žEzÞn?ý©ò!vr¿æњì¢L"¿×•&'¿âDîôàt¿î¶9ÀãWPSRPSRPSR J1745+1017?pp´X¾?n5œüJ,N?ïß—ÕÕP?n5œüJ,N?¢/m#-x²?­·,F´ö?îÝ	-Í(s?­·,F´õ?²c¢2íÿ}?¤Œ¾Ö÷?í³‹¹¢@?¤Œ¾Öù?£‰ÚÊ$?Ùð'¤•?îÎGo¢S]?Ùð'¤•3FGL J1745.6-2859c@vJ r~¿¤¾¿À`2À6	škP°òÀ8f€®I#?Ñ1뷕ûL@ä•Wëy`@'þ Œ=¿ç¥ìù'þu¿åõÁF†Í¿ß%áË·y¿åß äçuÅOTHERspp ?鈕Vê
?ƈüUZ†"?˥ݪ¤WË?ƈüUZ†"?æŽXWéë©?Ôð'L»‰Ž?ÒãOP,(­?Ôð'L»‰Ž?æ&³Ú¡Å?µGŽoiµ?ӳܘJ¼x?µGŽoiµ?ì1À"F?ÇÀ
‡Ÿ8¿?¾qûß½Ï^?ÇÀ
‡Ÿ8¾3FGL J1745.7+3952@Pd™àvp@=	› æÀ:¨KAFò-À;Õ«ïÝs
?áû=ЕÉ@
= åRՐ?ú÷x_7H¿æ£…µOòJ¿ë‰IáZ¿Ú)ҝ'n?Պ`·áêQAGNbllB2 1743+39C?ïûhGŠnã?NkŠ:ºÓ?B^áÖDq©?NkŠ:ºÊ?ïÊÿ§_'?ƒ¯/ƒLkS?zô,P7=?ƒ¯/ƒLkS?ïwLtOӝ?‰Té(P'?'qvŒ?‰Té(P'?ï¼aQL=N?'HÜg0'ï?€ç«¬ð¬h?'HÜg0'ï3FGL J1746.3-2851c?à ÖdP¿ºh~À5 ÝÀ6‡7`ÆÀ8·*´ßp=@áhy@-5ŠÑTÇ?óËá'LË
?í}Â"¤Å¿Õ¿Ó?,» ¿äè‰÷e&Ë¿êO© ø³…OTHERpwnPWN G0.13-0.110?Tvᄍ¬J?Rƕø€r?ïõď=¹*?Rƕø€r?XÅ~Så™?u៴/½?ïóù@Ö?u៴/½?"
@Ïi¦?"UÿÁZ"?ïg—Uù"²?"UÿÁZ"?ŠKì5òψ?ˆjĎ#èc?ï–ÐO(4Â?ˆjĎ#èc3FGL J1746.8-3240@vO¿Î·‰ÀH?Z³ÖÀ7a<ðKWÀ:0ñ>œ@×Þ§À£Ê@ú§S@™Î@o$¥ü©¿ß}wŸžÁL¿âL2_Æ«¿è™»L
´S¿í<ôàg3kPSRPSRLAT PSR J1746-3239?)} ô=þ? ~Ìu'«?ïþh%ð¼.? ~Ìu'«?61eõŠœ?T˜wÂ'ÿÎ?ïý9ÓA]P?T˜wÂ'ÿÎ?'ѳo€ç?yÔåc–¯i?ï´¹2AÿÀ?yÔåc–¯[?YŒ,YRîç?P¤ôÕ?ïó9éÓVŠ?P¤ôÕ3FGL J1747.1+0139@:õ€`°@.FÓÀ9n‡Êd<ÀÀ;©¿Š¯¿àl
‰_©x@Ò[]@%ù?œx¿å]yfâüÔ¿çv4ËÊÕ¿èŠW+±¿ïþ÷'ò[RAGNbcuPMN J1746+0141?îXçXÆ«k?«™;[ï#?ªqŠs•IU?«™;[ï#?íۋ¢0Ý?³E™•s[?±#¢îyH?³E™•s[?êü¶­È3?­'.£-¦?Ä
%KÐß2?­'.£-¦?ì¹ —Nm#?³¦3
Ҋ/?º6ûEŒ–î?³¦3
Ҋ.3FGL J1747.2-2958@vt´ ½¿ë@~ D¹À6rA&:ý,À9gåëoO@¾o›Cgß@bqŕ 
@yV-3??ÄéVäEíԿ丄&~Ÿ¿ç*‡ÿs,¿íœ‰8#PSRPSRPSR J1747-2958?KõŽbg£?DƒÉ)¥Ï?ïù<œgg?DƒÉ)¥Ï?1õ´‰¡èV?N|úÌhU=?ïýÁInËÂ?N|úÌhU=?"œ
Žçó×?"£íµßNÙ?ïc«ˆÀ`?"£íµßN×?^7A–èè?[EHàƒ?ïðä_4ò?[EHà'3FGL J1747.6-4037@uâî_ú;›À˜Ü )€­À8Ü4mÅÖ9À;8>4îõ?ð{"§;™@¶ÇÖÃƔ@•¡ŸÍeN¿¨—ÌöúY¿äìȜÄû¿äâCåe¨"¿ì
tñÅÄPSRPSRPSR J1747-4036?©=h‹ž?¬"Uv,ä*?îoÜ)wF?¬"Uv,ä*?Â
$÷ö?Çkr\:is?ë}vþ9'?Çkr\:is?Íåf
‰¯?µqñÀ]v?膽æ}]"?µqñÀ]u?ËYä¤<:¼?¤
çÎ4?é)†ÖðñQ?¤
çÎ43FGL J1748.0-2447@¡v m³¸?û€à»AÀ7VãÉW,À:$GŠLá@ö‡`±ñ@JÁ"àL[?øQO¶ñï¿Í¤‰øóB¿ÞY bvÞ¿äðè géô¿í( 2:OTHERglcTerzan 5?'*¥~ᢪ?'í»üüb?ï·Ujyv?'í»üüc?F˜¡"ÒEH?\B–ÔÜU™?ïúYךËo?\B–ÔÜU™?½°=ÊÚq–?±þÙk)-ô?ìIøF¤±Î?±þÙk)-ó?€…ú—Sçç?s
ΊtZ?ï½è¢°`?s
ΊtZ3FGL J1748.0+3405@M¬BŸ·ÀÌ@;.¦ÿ³©æÀ9œV÷]šÀ;É,¨Õv¿À(UR—Òo@†íð]÷@²ÍOÔ¿æ]ìÎ꽿ã—B•¿ç‡@fn'¿ÚI-è½æwAGNfsrqMG2 J174803+3403?ïõë{‡ï?]™J@b?Uæ)ð"}?]™J@b?ïÙ!,ù'8?€ÓêÁ?=?soiƒlcö?€ÓêÁ?>?ï[àî#,?Œª·‰ÊÜ?"ŸÃâ;š™?Œª·‰ÊÙ?ïÿï>€»r>î)5ˆq>àÁD?¬>î)5ˆÏ3FGL J1748.6+7005@Y!ˆ M@>µ 6×-À7͙ȓ'(À;#Ö~ý6!¿²µ¹¶'à@õ΋"Çs@ƒäŸÒBØ¿àtæu¯¿á'À¦<¯¿àr|Ý~ÔO¿áªÀÐë‹AGNbllS4 1749+70?ïÿ8+YK?	dô:›æ?ñõ)­nÐ?	dô:›m?ï×ߊÕW!?€Š+åÝ(N?t:•To?€Š+åÝ(O?ïʯÖ÷I?~†-vlæq?z¨"[|G?~†-vlæw?ïÿÿ©¢‰>«ñʙé>Ÿ
Ë®ìJº>«ñʙžU3FGL J1748.9-2021@÷ŒÕ£5@TRRá#À7éèEÏÀ:"vOèu ?ß²žDÆzñ@‰Õ®óò@aŸØ"¿ãÊc0Q¤¿é~ùÞ1¤¿äy–ÄÓH¿îmÁBá&OTHERglcNGC 6440?Ö¹"Ä'¦G?ÌaÑ´9Úr?ä£=¶¬Ý?ÌaÑ´9Úq?Öø¿2Œš‹?Ó.—Cë<?䃠f¹²º?Ó.—Cë<?àÂƋ_ÿ"?¹z°7þ?Þzré@Ú?¹z°7þ?×ðB£;s?¿
¨Wø?äþÞ®bG?¿
¨Wø3FGL J1749.1+4322@Qi # –@=#ì_9K{À9
AðeXIÀ;¬ŽÁÏBÉ¿ùù"Œº8 @úVÆz@ù¬ƒ(¿â‡½m֔™¿åUifK
š¿Þ4
LùǛ¿è¨ú_­AGNbllB3 1747+433?ïù²l‰b?Lž%³P€à?I6OÚxG?Lž%³P€ê?ïÊ-ê'?ƒãÉÄ?zé
ü·~Ç?ƒãÉÄ?îÑW.¤J??šÊuS­?¢ê»\?šÊuSª?ïüÊWm¢ô?AtD	çL?9­D'è_Ü?AtD	çK3FGL J1750.2-3704@v^ FÇeÀ+_ª4œÀ8³¼Àæ½À:éÜF½S³?ï|@Lv@
hhîV	@³Öà¡ëοâÓíçпåjÑfe¿å¸ÜP'`¿ìˆ¡ú'+6OTHERglcNGC 6441?¡n~Ìá5?¦ûàpqa?îé1ì¨?¦ûàpqa?£Â>*–s?´í¬kK3Ñ?îÃÞ,V™?´í¬kK3Ñ?Ðí]Æö?¶8)ë
'¡?ç‰Qñð…?¶8)ë
'¡?¼1¯õ;3?žÌ"&þP¢?ì|ùÊXš?žÌ"&þP¢3FGL J1751.5+0939@Avf H	"@1¦ý`OÀ7ù¢(´T0À;l5ç?úåÙ¡q@|Z
w¢@5÷Rñj¿Öp†Ҙ¿å=WÏ¿ã Áõ
¿èî>D´AGNbllOT 081?ïäqp÷Q®?w‹…b¾$?kŽ®PÕ?w‹…b¾"?ïÊj‹ƒÉS?'–²nÕÝe?zʺ>VÐ?'–²nÕÝc?ì6-'Zææ?¨9ç˜rÅ?¾N"m(ÈÉ?¨9ç˜rÅ?ï:áÝC	ç?ŽjI&YÊ5?˜£ÄWžÃ3?ŽjI&YÊ43FGL J1753.5-5010@udvâ—À'ù¶^À9Jûüe@ÌÀ;^&>?Ԁ‹"ò²S@9DM·ÃÑ@(Ððž¿ßk6cƒ ö¿ä뜋ýÈ¿éÊ°¤o¿ïÿÇo.¦AGNbcuPMN J1753-5015?ïí•ÅŽî°?hÕhÇÊ?bj:qPi?hÕhÇÍ?ïÅÐLð¸"?‹"ú¬…ø<?}ه£¾;?‹"ú¬…ø<?ìù}Bãm?¥8Ž3Ú?¸4èç̓?¥8Ž3Ù?ïùWº4æÞ?D迯Tv¦?J¡,d‹×?D迯Tv•3FGL J1754.1+3212@LÞß¿î—ù@9j´M,ÙÀ7ôkõ oÀ:áNÊϝ?êÆ"Ì¿@Ú¾[?þl>ÙÚ¿Ýö?ý›÷˜¿Ü3
Ú¼¿ÚþE(‰Ñ¿Ýï¯f"AGNbllRX J1754.1+3212?ïþÃ¨".?%-G³}V¦?&#Åv½?%-G³}VÆ?ï×J~™á™?EÞVh×?tZÀ³3ö?EÞVhÙ?{q;û?~B²±X?€™#±9Á]?~B²±Q?ïÿ ¯­E‡?'éz?Ô®žD²?'éz/3FGL J1754.3-6424@t'ñ@ìFÀ2r?©c;À9Îw/†FÀ;­±¨"(?Óº0q.@[¹ïÐ\ú@«r`o¬`¿åø¬˜5&º¿äâƒ3ëXÿ蚓Ð4"ä¿á£¯ƒAGNbllPMN J1754-6423?ïÖª'=C
?y™œÀn:?tª·a^y¬?y™œÀn6?ïy'ØJn?œqYp€?ÍÄö¿Rc?œqYp€	?ï+œdZoØ?'wDö
?šŒst²ø?'wDö
?î·»A;K?•'v'žyÞ?¤"O;ìKI?•'v'žyÞ3FGL J1756.3+5523@TßÞÛgš@=·™€o&)À:M‡rO©À;áËÜñ?Þ[ǤÍ\ó@o»îƒ*í?ÿ°ð`$ØÒ¿Ø/óÃ[´Ý¿ìn`mŠ?¢A>lTð{¿Ï÷Xš¼ýAGNbll1RXS J175615.5+552217?ïéŸ:~¼?pDnt¾Ès?fþ`ŁD$?pDnt¾Èu?﯋G÷?ŠQžÉÂ?";®8F?ŠQžÉÁ?ïPÅg´?·=
‹?•ç^	Œ?·=
…?ïS®Z(J?@´©ÔM£?•Š4ºüV´?@´©ÔM¤3FGL J1756.9+7032@Y?'à°«@=ûßä׆À:Á#å¸VÀ;üˆµENJ¿äó|îí@§†³bîb?ûIÇÚñS¿í8~_\¿æ´
ýÁ§¿ÒÈ ukg¿É…\¾ÐhkAGNbllMS 1757.7+7034?ïÿs °$?S.:eŠò?Ÿ{éûyQ?S.:eŠÉ?ïÓÿÁ$?€XÂՊ?vmövÈ?€XÂՊ?ïÇbÉÙ?{g?Sð‰?|rNÀ?{g?Sð‹?ïûbh®Ù?A"m¦t?BwÎ]D¥?A"m¦ˆ3FGL J1757.1+1533@D–uŸ¿Mˆ@2ߏ`Z³«À:-LBα©À;ŸÙ0ˆ^?ðY— ñ@q•înr@\"Dž?嘖Ät†¿Ø·§.¶){¿Þ™À&Ä¿ïÿÞ&çJ|AGNbcu87GB 175437.6+153548?Ù¦–`œcË?҃Kç}¡?ã,´Ï±Î?҃Kç}¡?Õ>Èv–?ÑM]¼Þ7m?åw`›Äõ5?ÑM]¼Þ7m?Ú7ÑÉ
?ºÿr)҆Å?âäs~y?ºÿr)҆Å?օm
·´?¾GxÌ;?ä½{Éy$&?¾GxÌ;3FGL J1757.4+6536@WÑÇ@0q¸@>?ÐàÀ: À
¡©À;þÀ°^×ý?Þ¦mV^u@¥'Ð&Ém@‰ãŸÍh¿é*š=¿ê[Ôþ…½«¿ëW°év?ãP0…•AGNbcu7C 1757+6536?ïóQV«;û?`	²]‰R?Y]R©ˆn?`	²]‰H?ïÊáœwW?'³$I´fô?z1ÄT|´?'³$I´fó?îKI‹öñÊ? ³R€µ	#?«Kg@ãj? ³R€µ	$?ïצ'ÙO?y €§Ä`=?t,¾úXC?y €§Ä`<3FGL J1759.1-4822@u…|€"ÞÀ'ê"ßÎ1QÀ8þXÒ)- À;S&ìÓÓ?â×Hêæ¤u@×E¼wÀ@^%à9f(¿âö¬…ڿⶰdGŽp¿æ7ƞñƒw¿ærI@¾ÕAGNbcuPMN J1758-4820?ïçYÔº!?hIAeÇÙ?h¦+EæÞ£?hIAeÇÜ?ïÂ0Fó¡/?†TܙQ¾2?~ç܆/h¦?†TܙQ¾1?î5*I P? œªBÈy?¬­^›mû
? œªBÈx?ïùhå—6Œ?A:äx-µ±?J\i£%Óþ?A:äx-µ'3FGL J1800.5+7827@['~¡Æ@=×ÿ/öhÀ7[M-°<À;>*ðn'…?"­B@EOÐwÒ@È@3KÝ¿ãnÒ]Qâ¿ã¡Â¨0¶+¿áÁ	¾«Ýû¿ä×¼Öú<AGNbllS5 1803+784?ïÿ£îÓ?}ñ'V©?z‹‰^?}ñ'WR?ïØz–­?×°7VC?sÂö´©xf?×°7VC?ï¥êƒÀŽê?ˆÎIi'­‡?†…_ÜE€?ˆÎIi'­Š?ïÿçKV}'>ñ3ő"­>è´©'n‡}>ñ3ő"‹3FGL J1801.3-2326e@¬ÐDÑ¿ÐB OÅÀ5™þJZ"À9lžéd³@w¹ŸôR@mÁ̾Š?üßÎoU®¿ÑNŠ§ŽNã¿ãoNlt¿å;ÇÁË¿èÙRav½wOTHERSNRW28?Ïv™'R?Ðá™Qt²?è"zٛ¼j?Ðá™Qt²?MR΍ßâ?|=œAwê•?ïø˜«L\‡?|=œAwê•?؞»¨ÃK¸?½ááÑý"Â?ã°¢+žZ%?½ááÑý"Ã?q]Ù>Áë-?q9£ŸŠ-V?ïÝDM'|*?q9£ŸŠ-U3FGL J1801.5+4403@Q»&ßÓ9Î@;þßnÀ9g½¨l›4À;ÍVØS錿ҐÑ4¡®w@¶6b½m@`M˜¿æ…$J?ÇÊ¿é¡[j'xœ¿ãéUͬW¿ïÿY,t°µAGNfsrqS4 1800+44?ïÿaK"Gò?€gë•Ú?֏wÕº?€gë–‰?ïq¾}Ób?"áƒG'UÔ?£`‹'Ø?"áƒG'UÕ?ïÉèjÅ*?wKôPÖýû?{Êôjê?wKôPÖýó?ï°EûEÝ
?|±‹þ
?ƒî.ˆ¼¤?|±‹þ
3FGL J1802.6-3940@v`—ÌÀ ٍ0À7?ep!À:žT~ÝU±?ýaÛQÊÍï@ç%=§*@ñVe'V¿ß·w=ׯ‡¿ån~P›"¿äEdNM¿è ÑxFýYAGNfsrqPMN J1802-3940?ï¾ô`:aó?'Žï}ZÃ?€Bçñg'Ö?'Žï}ZÃ?ï4&õ‹™¬?«ºël­?™{!NŒÊ{?«ºël­?í£¿®PE?¤.³)­ß?²âU}Õ?¤.³)­à?ïþÒ—8?0%ufʇ?"Þ¦ŒxÅ?0%ufÊg3FGL J1803.1-2147@ U,î‡Þ?ÊÔ)`T18À7!DҗçéÀ9º[‡SZ@ªu
Iè@¥öy|Ä?ùÍBM­\ð?ïýǯ½®ˆ¿à*Cùb¿àÀfÂ#Gû¿ì¯–kÅSPSRPSRLAT PSR J1803-2149?VϾ?ˆÊ'ψÅÌ?ï»Þ§œÁ?ˆÊ'ψÅÌ?NkIðO8?k"sjYš?ïøe-ƒì3?k"sjYš?¡¹Ñpֆ?žLû©Y?îçbèò–?žLû©^?ŠQiÜP‡?'}ow¸É?ï—ÒºXŽ½?'}ow¸É3FGL J1804.1+0341@>Ô}`}ï@(h³Þ¿=˜À9í´ùqp†À;^èÅP׉¿Ô¹öP©»¦@Ò´WàçŒ@xÀ†‡¿ã' »Ä3C¿å¶ŠE"²û¿ß¿
º9¿æ›kFÜ«AGNfsrqTXS 1801+036?ïÿ›f˜ŽA?qÎ4óE+?	&YÜoÐ:?qÎ4óF:?ïÛ®£ÚV?~+çøëÃÀ?r(®Ô¾?~+çøëÃÁ?ïÖÃ
Uø?}ߪçÃ"0?tóyU.?}ߪçÃ".?ïõ»)¹?Ob,†Œa?TÅô‰¬Î?Ob,†Œa%3FGL J1805.6-2136e@!5\ ¿Êû@?W¦'À6O«ºbgÀ9yºZÚA*?ü>ÐJZÂ@ì}'%VÒ?ü³~'W0¿Ò"ŸÅÒ=¿áñëjFÆ¿âõѨԠ¿äóEšOTHERSNRW30?蘲ù÷Ég?Ê[‡jæœ?͝4 Úb?Ê[‡jæœ?¡Ñ'š®×?¶'ja
ØF?îâçÖU?¶'ja
ØG?ãՅ[8?·Ê\[Ÿ<Æ?ÙTõIŽÇ?·Ê\[Ÿ<Æ?ÀCžê;£?±îÓ¾ChÂ?ëïEzq?±îÓ¾ChÂ3FGL J1805.9+0614@@­çÖyõ@)矾vÉÀ9ìŽÐè»@À;£ŸM7Á7?÷x&º©ß@
'ë¡?Ë¥Öé±4?Û¨¢þiŸM¿ÈÁV8¾.ò¿à«ñ«uÜ¿í-b
çPSRpsrPSR J1805+06?¯ÊË£ºy?É`¥/2P?îSEÄXh?É`¥/2P?¢§[ÜöÔ?¾œü˜¡ß?îՎ
B0'?¾œü˜¡ß?²‹€jË:ð?«YÏ·1o?í®ò¦˜¢?«YÏ·1o?®)6'Øÿ?§|Ÿ¾ßãp?îoœ–Òn?§|Ÿ¾ßãp3FGL J1806.7+6949@Yñà'Œ7@=-SaÅÀ7÷Þ¡
§#À;Zë´ï`v?ð-3¢Câ-@^!p¾0@ßGŸ¦Îá¿Ý‰V)q,W¿äp¡1'GÝ¿ãOK Î}b¿äë]ö͞¦AGNbll3C 371?ïþóÖ@^?$È	!ú¢¤? žKú½?$È	!ú¢ó?ï¼ÑÓ¦6~?‰K
ÑÂrß?€Ë‹r`?‰K
ÑÂrá?ïJad?d®d_±Â?–¾œ"Ó|‹?d®d_±Ã?ïŒ%!q?…y!Êh?Œö·¸<#…?…y!Êh3FGL J1807.5-4343@uÓÞ²gÇÀ&9@LzÀ9è6°–5aÀ;xcNƒñ'?ñ&>Þb ‡@î)#øÁ@ö<À$È·?Ñ$Š#¿ÔBÖÿ«œQ¿á~?kOÚ3¿ïÿÞý¦ßROTHERglcNGC 6541?À'"T#?ÃXÖîSz?ëø›šê÷??ÃXÖîSz?¨T†ZÈÑ9?»¦GR»?îz·šSrí?»¦GR»?ÍÝJ'Ýã?·[P¾ÕN@?è½­_H‡?·[P¾ÕNA?ÂGo~J¸?ªwÆ6;í??ën$ m|R?ªwÆ6;í?3FGL J1807.8+6427@W†À
¡©@<ó?ÀàÀ:žQ>ÌÄÀ<èÙrÍ}¿õ"§èö@Dt¤@½_€C1X¿É¯…°꪿à*:ø4Á¿â0@ÔÓÎÁ¿Ø#hÖ¿PAGNbcu7C 1807+6428?ïð,w?l…PÐÊ3H?_éõ§ü2?l…PÐÊ3H?ïØ 6÷?~ÒøUü?s¯ä"v93?~ÒøUû?îçÁÐ,?i?ž'ê-,|Ä?¡ƒâý<	b?ž'ê-,|Ä?ïÿµ€ý¿?L\Öw‰?ŸÀ»Ð°$?L\Öw3FGL J1807.8-5011@uuIàâiÀ,?{@À:¦Ë±DÀ;xût€¿ìäkWšy@înKbª@X+Àx*´¿â%Ÿ¿èðj¿D,¿è ·§exï¿Ë†)žÎ¦…AGNfsrqPMN J1808-5011?ïø3̄1$?QúÛToœÂ?O0Íï;kÔ?QúÛToœÐ?ïÙW}™?€·Ìb½ç‡?sT}Á³e?€·Ìb½çˆ?ï•q[«j?…¯ý rÈ?Š£©:%}?…¯ý rÇ?ïþ⊽ê?ê¤×rëð?!×T!_±e?ê¤×rëæ3FGL J1808.0+4652@R'³`<Î@:'
4fÀ:ÄIqcÀ;ððÄXŠ¿¶C²"b¼Ÿ@¸Šh#Tï?û¤h_dêe¿ïyATõP?ïi†âðµ¿Û+ý¥Ãڜ¿Ó'ë=Œc·AGNbllRGB J1808+468?ïû¶ï?G'Ô˜7¦4?B'ï˜Hž?G'Ô˜7¦-?ï¾2¦vŸf?"?²é]¢?€sVbX&¡?"?²é]£?ï©ÓµiÚ?'à•5nT2?…ºK¥‰š?'à•5nT8?ײַcüjÚ?€Qð\MÞæ?"Ø'åIn?€Qð\MÞç3FGL J1808.5-1952@$ê;¡–¾?£z"`h®<À7֓vié©À9´rcÊ«?ù¥)Gwý@¶ktBG"?ým¤ˆµñ"¿ä»?܎â¿Õܾ²Wց¿çíß¡»§¿é!& þ'ÃOTHERglc2MS-GC01?R›¶p—î?SÝóë^Dñ?ïö²$Ç´t?SÝóë^Dñ?87–óó%?–Ë,ÞÄ@?ï»!¤03?–Ë,ÞÄ@?¦›­«âP?¤Ž>û]¼?î–E%AÛ?¤Ž>û]¼?«Ý‹lkŠ? (á€\Q?îB'I?éH? (á€\Q3FGL J1809.4+2040@G¬Ì W"ý@2:X@2õ÷À:2@ºˆ'À;¥:Ùâ)?ÜR!ñþpÅ@
·‰Ð£Æï?þ)¡-¿ä¨©¶—¿íõfß捜?ݜ—¡ƒ;¿ÆìàϟKFAGNbllRX J1809.3+2041?ïýŽU¸/?<™ïƒd<?3R?NŽ4?<™ïƒd?ïÛ£`K	?}åÅ$Æ3?r.}ÏÚ{Ž?}åÅ$Æ0?ï­<ò¼¼Ì?ÐòÀ7ϙ?"°ÃPÐÌô?ÐòÀ7ϓ?ïî(2œ!Ì?h§ÀC9bî?a×ÍcÞ3º?h§ÀC9bë3FGL J1809.7+2909@Kás 
Ìã@5F(ÿӊVÀ9
3èdØÈÀ;Lü~¹D?剞C™Õ @×Ú Ÿó?þ}a?5¿Ûéß¿Ø
‡ñ"޿ۊIþYj]¿ÜÜÇÊ7$AGNbllMG2 J180948+2910?ïùç~J?D:	Ÿ×6\?HñbšØð?D:	Ÿ×6n?ï¾SEÁeG?†ŠvB»V}?€k.¦®S?†ŠvB»V}?ï¡-o÷ãH?†Ž¡‡:ìü?‡´¤-Ø?†Ž¡‡:ìþ?îö¼AC¡½?‡ ÇÈ`R? ";ëÅä*?‡ ÇÈ`P3FGL J1809.8-2332@^_±ÁYÀ˜Ÿô|"À5†·¯.VUÀ9Ñ쌅´à@E»ÕX·|@MØÈÙx,@®'oXÓV¿Õ.™1%"5¿à¤Øðz/¿å6KÕQ¼Ç¿ìÆ'ŽmÊPSRPSRPSR J1809-2332?$ìђä? 1"]š?ïþ±>ÃÆç? 1"]š?"øv]–]÷?DºUÅ)?ïþÐxš&š?DºUÅ)?sÝ[á}6?`í—õ44‰?ïØEIÞ=?`í—õ44'>É­+¦õ>їL#?ïÿù"»˜¶>їL#3FGL J1810.1-1910@&">'âÆ?§Q*?ô«œÀ8w~@w¿TÀ9ÄõǗ٦¿ý~™Îr¿:@œˆjÈê@ÅT`)‹j?ïKæ'øm¿êý
!P² ¿à9õÅšç¿äˆc`øh\OTHERspp?ìÿpã"	º?½ñ£Ó.ê?¸xãg²#?½ñ£Ó.ê?íJc£±¹O?ÈցaXú?µ¬ââr5Š?ÈցaXú?ç"Eý
Ɩ?³Þ§#Shû?Ð×tärÕ?³Þ§#Shû?ïþ]êD¼?Bû¤ŽôT?*![·$@?Bû¤ŽôT3FGL J1810.5+1743@FNÌ W"ý@0Îs`Iì³À8…Í!†b…À;Q€J=:ô?ýû%Þ
¥@––'7þ@ÅN¢zhÒ¿à–X¿äjlÊ9¿æÒS¬âˆ¿îùU=8ŸPSRPSRPSR J1810+1744?'ÏíGI?'8Ä"üb?ïw§é€•Å?'8Ä"üb?•2ÖuPŸ?¢'+\ýø?ïViLUC?¢'+\ýø?´O€©K9®?ª"%QV*?ívê֘Ê?ª"%QV*?…y"@å[?w'["?者üiù?w'["3FGL J1810.8+1609@E"©Ÿ¡—@0$™ù;À9Xˊ­mŒÀ;Zˆú%7?ãp+¶s@#»DLÊ@ۇß\òI?ëLøWÙÊ{¿æ/™"9ƒ.¿Ü–æ°N¿æi$nÔ AGNbll87GB 180835.5+160714?ïôTïïh¤?V}Ç»Ê\b?WV !.¹Ñ?V}Ç»Ê\_?ï~ê^2i?'–tBÊ)'?"´9¾2÷?'–tBÊ)&?îÜîÛ=™-?˜3VÝö?ñ?¢1L&m>?˜3VÝö?ï?í¦ÃÙér"?›ïm)e1"?²Éá0´kn?›ïm)e1"3FGL J1811.2+0340@?¢æ_E	õ@%8žç·4À9Hê7.jÀ;"nÞ,µ?òî«¢°š@b}¤ñfŠ?û\zßð&?ïâ]¨QÃA?ÃT…µ®oŒ¿Ð}‡0Fªð¿àå…é—†AGNbllNVSS J181118+034113?î;'+ñ?¯wȬ'Pt?¬FíNoÀç?¯wȬ'Ps?íX'xÄž?ÀÇü=jEê?µ;t9ÙÒ?ÀÇü=jEé?ëóbøa?«¸‰d2??À3Âtr?«¸‰d2>?é0øù
Çt?¶OF®L?Ë<Ôâ.?¶OF®K3FGL J1811.3-1927c@&Cù¡A-È¿Ôñ·€
IÀ8iǾp¸À9¼ÑÇÞPƒ?ìÓNà҂@לã{@áŠÿ¢âî¿çOhË?ç~œóÁ-\¿áú©êIµV¿èpË¡ÖªOTHERspp ?¿_úìå é?Á^vïΧ?ì¢cKã?Á^vïΧ?Õdùr{,?Ôm²_ú?åMƒFÂiú?Ôm²_ú?ÚcӞ…'ø?¶öGØ%ÍB?âÎ0½l?¶öGØ%ÍA?áÍm•¾N?ÊÔõ%!?Üe%öԃc?ÊÔõ%!3FGL J1813.4-1246@1>`ºTû@ˆ•_ùõÀ6¹"ñkéÀ9àЉð@±CÄÐÔï@ÜúE€èž@68õ¿à*¿Þû‡Ë:ü¿å"P3Áoï¿è @*8n¿îE;­nýSPSRPSRLAT PSR J1813-1246?8tf­Oæ?8j~¶ø—·?ïüñs*V ?8j~¶ø—¶?2UB0*,±?J«JRÈk'?ïýµW¹ú»?J«JRÈk'?£â>bÖÉ®?›AnøFÕ?îÁÜғe?›AnøFØ>õáÚ-€­Ý>ú«oÍtA¹?ïÿÔ<K¤ý>ú«oÍtA¹3FGL J1813.6+0614@A»®²@&x¾áQ¿À9JEµì¶wÀ;:,XN?í¡Ô¬rÂÉ@st¤íŠ²?þW@-†?ï©
o6¿ÃWû'e¦V¿ÜPMR÷§J¿áî2|÷CæAGNbllTXS 1811+062?ïûÐrn"?DÓy­žx?@¾6E³†ç?DÓy­žt?ïl	ü¢ž?¤ž}ìã–õ?'~Àk¼¬g?¤ž}ìã–õ?îωsñi?˜™\"§—ÿ?£nÀéf?˜™\"§—ü?î+Q+?}™ºC:?®ÍNªïýR?}™ºC93FGL J1813.6+3143@MU§€)Ú@5Y‰?¯BxÀ95†S€À;…¿üñý?õÐq‡¿@ð`±¿Ÿ?ú­ròe㊿ÕWøÿi¿ß¯ˆ:Ãí¢¿ç(´Ù¿àÇæ|²iZAGNbllB2 1811+31?è^ê:‹—?ÇÎÌð'À?·ìWѤ?ÇÎÌð'À?ê-èÜæç]?ÎÚtt<?ÇH\Œdb†?ÎÚtt<?çÛ±Px]?³†Uú™?ÐH_ÕD?³†Uú™?ڞ«¡`;æ?À6òÒ?â°ª/Oâ
?À6òÒ3FGL J1816.5+4512@R6¢Àh¡@8Àæ_E	õÀ9"¤úö«ÃÀ;µ(Ùº?úDن@p…qœ@äe½Ÿ¿×-ó´±è¿à0Pÿ³0¿ãꯋ?Ü¿ìÊ9­~[ƒPSRPSRPSR J1816+4510?Ce­þ5*$?E="í+á?ïû&"€r¶?E="í+â?‰{,¸td‰?'#[úàuï?ïšM.p?'#[úàuï?š$¯P®£?>&¾Ú=?ï.ڇMz‹?>&¾Ú="?ÿ$iª$?€ÐԙÉ+è?ïx>ܲ­?€ÐԙÉ+è3FGL J1816.9-4944@u† fèÀ.X­~«À9ülhÞæ«À;Ë?'‡]?ö
´ynÖÍ@·Ýª»ú?í{xg«ñò?ïGãmðjÙ¿Û0!œõ¿ååÏA"•–¿ïþ'B)'˜AGNbcuPMN J1816-4943?êæµÜj^?Ç~;Ðä¢Ù?Äe(ŽW–‡?Ç~;Ðä¢Ø?ÑYSÃ\>œ?Ô{Vú˜¥?çSVQà³?Ô{Vú˜¥?݀'˜Õ	¼?¸…±hšì?á?ì3•{"?¸…±hšì?ß4~W>³é?º"àÊM?àeÀÔ`¦?º"àÊN3FGL J1817.2-1739@*Ç$ß³Y^¿æ-£€Š#À8@5¾þ­ðÀ9î'Iü?óEêmFª^@ŸŸšm@+/ŸÕÈÊ?å´õ«gâ¿æ˜"üS£¿á8½`É¿èš´¡²ÂµOTHERspp?ÉZ¹iÇ?ÈL`kԖ•?鹿iQ¥Ž?ÈL`kԖ•?݊ß>èe!?Õ¶	Ò|š¯?á:`‹Ío?Õ¶	Ò|š¯?Õö Ïï?¼	yÓ#u?寘wó‰?¼	yÓ#u?åpÃb¼9?Å1ƒLZ?Õy:‡Å?Å1ƒLZ3FGL J1818.6+0903@B¯¸Ÿï0@&¿ãAƒXÀ8¾Š¯ñʳÀ;0žHUh¿íû¨V@wEöÚ<w@ð6îÍ©¿ã69Àk¡¿ãÆX¶È¿ç.«'5>s¿ã+h¸óswAGNfsrqMG1 J181841+0903?ï÷Œû#ÛÉ?Qòú?¿'ž?Pæ	¸Hló?Qòú?¿'š?ïٖIµÅJ?{+ËL,²Õ?s4Û%\?{+ËL,²Ô?ïEM"+^¬?_è躙à?—VOz"*Ÿ?_è躙à?ïúvô2%´?DB¶M'´.?F$/7i5?DB¶M'´3FGL J1818.7-1528@.ù"!bPW?ƒþèÀ(½¤À7söLø×À9 Š(Ž"@þê<F'@Ipû@?ýr9΂Úe¿ÃQ²º§Ü(¿æ>ÕÈôÐø¿è¼*2	h¿êÖ#ú±OTHERspp@?ÛÆÙÔrS¨?Ðx…¦'?â"ÆÖ+?Ðx…¦'?ªPÆjÈ®¡?»S£'¦?îZó™Su?»S£'¦?Û´?Èl7…?¼su&Ê1?â%àÉä>?¼su&Ê1?¶lÞÅD9?«@à¹?í2}'Wy?«@à¹3FGL J1819.1+2134@H'ŸÀ$GÞ@0}>ö?À9å(¡ù¤À;Š¦8
‡¿¼KŠÔ&¿@'ÈVñSj@¨_Û÷¿á֟ÞÏ{¿ãè½YDóX¿äv'6+"µ¿²^B¸XÃÞAGNbcuMG2 J181902+2132?ïäè¦q?tFZ̋É?kYŽøý&?tFZ̋É?ïܾ>ë¶?z$Ç'IÈ?qô àŠ$³?z$Ç'IÇ?îó®î8J?™ôLqc~? Å~›T?™ôLqc}?ïã¼ä?bú«ºg?-?läáCý©?bú«ºg?*3FGL J1819.1+4259@Q©'ŸÐ€@7¸ß_vˆÀ:<³Þ¿=˜À;ΌQ²z;¿Öô&žáhK@¥²YY·@߃]ÿålòÊÀᐿî'ÜDÓ³`?ÚuYÂØÆð¿éü½ðˆ`.AGNbcuNVSS J181927+425800?ïÿ°'Xj?›s n¸Ù?‰ï´ò"?›s n¸Ï?ïÕäv«£?Fô>‰@þ?u
Ī1.?Fô>‰@û?ï'Áã1¡Ó?‡©¸lÌt?‹O‡3—‹:?‡©¸lÌq?ï÷p¯×â?c–ÓúÀK?Q P;ݸ?c–ÓúÀKŒ3FGL J1820.3+3625@Oõð ¬ @5'â_ܪÀ:m&!Ò¸ŸÀ;ÓùrGE¿ã>ªCF7@x¹ÖÐܧ?ümá?¥¿æcÝ	ñ_¿æ¶[[	f¿Ö'÷6‹_ù?¾d´AˆAGNbcuNVSS J182021+362343?ïÿ|$ÉÆ×?¼ÉmQXå?{fÇ%Nñ?¼ÉmQX:?ïÞ¬,N Y?x½Þ›ÈÝI?p©éدÓL?x½Þ›ÈÝG?ïàÿ-ðR?js›WO&?oæÒ­q?js›WO!?ïü»S¶$ê?;~¾ [?:%bNØ´Ø?;~¾ u3FGL J1822.1-7051@t:gÿyÈÀ7.L`*ãÀ9õågÎEÀ;«¸ÕŸf?ÆG^™‹@EôZƒG@Ÿ¦ e¦"¿çµ¾t´ È¿éJÐeUË¿æ	c3´–¿ïÿƒ£žÃAGNbcuPMN J1823-7056?ïîZΞI?rUÚò#Ý?aì¥1a·'?rUÚò#Ú?ÜV²—G3£?ÑKOMB0Ž?áÔ¦´\f.?ÑKOMB0Ž?í®úë{'[?¡ô–­™)Ï?²ˆ(¤#í4?¡ô–­™)Î?ܯxc?À.tÉ>Ø6?áñ|¨CÎz?À.tÉ>Ø63FGL J1823.4+6857@XÌm_êKc@;­5@S­&À9`žc,öÀ;Æ\>'ãÀ^ÙH0Em@¬àÑ;œc@DI€§…@¿ä™Wž'>ñ¿åFfËÞ\º¿ÞZ'qf¨3¿ë!Hï ùAGNbll7C 1823+6856?ï"Ft¯®? ~7jéÍö?Ÿow1j
"? ~7jéÍö?ï× ٗX?rÒ§¤
?toõ"4S?rÒ§¤
?ëÃ*sfK(?­þUál:á?ÀóV2fÓ]?­þUál:â?ïÿ¹>Уz?¬ƒ…®«Ù?°K×!6ò?¬ƒ…®«Ä3FGL J1823.6-3453@vjá€M˜9À#Þ\ÀjTÀ8ƒè!¼é*À:ۚânõ?ì÷lN˜ûu@àóÇ™?ûùI þ?•jy³íz¿Óoò:îé¿Ó¾Òƒp'¿Ý«xÊþ&ÈAGNbcuNVSS J182338-345412?ï&þëÒÑ?›÷˜_x¡?› "…¼ó?›÷˜_x¡?ìç‹ÅøáÏ?ÀL'bWÞÕ?¸Ã¡Ð8ñ?ÀL'bWÞÕ?î5-&öô?Ÿ™¡ÄSÅ?¬­-žÖ?Ÿ™¡ÄSÈ?ìEVÛïu?§_<Ä6ª?¿ÕI "P?§_<Ä6ª3FGL J1823.7-3019@'œÿT´bÀŸ!€nÅÀ8ÜMÂ*²[À;&œKû?ì)¯‹žY@
þ{uí@yoÿl\J¿Ò>ÕÁp«Â¿áôôç0¿ä8úC8Ë	¿ê'ÖwŠ?PSRPSRPSR J1823-3021A?Æùèyš
?Ãye-aH?ê{Á…á™}?Ãye-aH?È='8øâz?ÎDŽ•¯Ò?éð›qÁÇa?ÎDŽ•¯Ò?܃õæ6æ˜?º'ìÎx(¯?á¾䌳?º'ìÎx(®?ÌÐ&Vïi?«21+J<ù?èËöjD%º?«21+J<ù3FGL J1824.0+1017@CŒß€-·É@%g‹_D36À9®TDZ±À;a~B%>~?óîÔâø@²¦Ú?ÿ×>€C\K¿·O£°•Ä¿Û»vžAôí¿×agnN<N¿îQo3òÿDPSRpsrPSR J1824+10?•Ü‡9–¡?š±Vw›M?ïQÆ7‹M?š±Vw›M?Ú^g{֐?ÑÑ¥$è']?âÐ÷ÌB¹?ÑÑ¥$è'^?Äÿ6r:Æ?°ö䎨s?êÀ2c±O?°ö䎨s?Ø=vó"=?¹Hêɍ«?ãáĆ6b?¹Hêɍ«3FGL J1824.2+5649@UnGßþù@:ÀÁ%ÐÀ8Iò×sÀ;‰ùÖñý?趃Q¹±@%͙ü@@®?Æ ¿ääÛ3a=¿åŸÿ«±¿çQIß/¶¿é‡pu«ÒAGNbll4C +56.27?ïø=—Eþè?K"lqòPr?O	¢è^¤?K"lqòPm?ïÓmÕù~?÷òêûî?vI@÷ ?÷òêûï?ïSYviÁ2?Ž¿õ)؇?•"Ñ2Çِ?Ž¿õ)؉?ïä%9íD»?e´¥Ö?kÚÆ»Cð?e´¥Ö3FGL J1824.4+4310@QÇß 'á@6ÙÙb¶®À:Íú8?ânÀ;øIlÊ.?ӕˆª€i@
"mã]\ý?û˜ÔÀ6;{¿ïÐwwclj?ïëé‹Û|#¿Ü P¤Õ"N¿×Œ0Nk6ÊAGNbcu1RXS J182418.7+430954?ïòmZ"þ?[&s˜Æ¸?[ã%JÖ¬?[&s˜Æ¸'?îÙ"OŽ?·Ìº9Ç î?®Bmß{ü?·Ìº9Ç ï?ï…Íÿ¶k?ˆH´YÝÎ?ŽŒ€8Reg?ˆH´YÝÒ?ë0ýV}¤?¶õçâ~¸?Ã<
¦ér?¶õçâ~¸3FGL J1824.5-1351e@1'A@<02¿Ý`às%oÀ6Œn~bÜnÀ9*Š§ŽNã?öWvšÙ@'
äµvÅ?ËÝJ9pJQ¿ØèPKqîZ?é«\ÚÌiÐ?à(‰¡~ëC¿Â²_8IÈOTHERPWNHESS J1825-137?РOYFË?˹½/¬n?ç¯ØS?\›?˹½/¬n?Ñ´ó)#K)?ÖlÕÀú?ç%†knZm?ÖlÕÀú?åí||´?²ÈCÔ¨º-?Ô%–åÆ?²ÈCÔ¨º-?ãõÃ
hå?ј—"d?Øyë/þ5?ј—"d3FGL J1824.6-2451@DHÿÎ+òÀa'ßÂó°À8E3å	ÚtÀ:Û5ƒo‹©?ü×È j® @ ½Ã@@"4"¿Ù­`Ç|<"¿ãs§ªyª¿åýÎl+™®¿îb!%û£`PSRPSRPSR J1824-2452A?-±µ¿×zw?'Ú	1)É?ïþ$䤉?'Ú	1)È?hã3)=?"rD†ó¹Ä?ïçÌÖøÄ?"rD†ó¹Ã?‹T¯>±t'?ŠÓO†?C:,?ŠÓO†?z3 £m·S?gíТƒs?ï˘¾¹$'?gíТƒs3FGL J1825.2-5230@udS_ôöÀ1w?› 'À8Óû|ÀÙÀ;Z*¤ï82?õŸ©X~qJ@óE$Í>ã?þTK'ôà¿Ñô]%†2›¿ä]rÍä
<¿æ˜ëK#¿ä±Çã%AGNbcuPKS 1821-525?ïôÙ~¢ù?W²µRkFˆ?VMôº%?W²µRkF‡?ïÃUqk_?‰°"°ˆ?~U~ÇJQ
?‰°"°‡?í¥f˜·kI?¢jWe†?²ÔË:D¥¹?¢jWe…?ïÚ|øÄèk?in9³Œ?rÁƒ‹Ê?in9³3FGL J1826.1-1256@2Žwß4®]¿ØJä@m»À5š'3K†çÀ9y[ñ˜^@	o_F6›@™åX3ô@ÃTUýŽ¿ÕmW=mc¿âš !¯¨¿æ嵕3êy¿îj+.¤O¢PSRPSRLAT PSR J1826-1256?/(†
XVd?#
¸·´)?ïþ
wŸ*{?#
¸·´)	? 3òÕZä£?5þ	óSº?ïþüÀÒªQ?5þ	óSº?t! ŸR¸?WAÿ.W?ï×¼¾Áý[?WAÿ.&?
õ÷¯'j?ÑØú…?ïÿ§È(!B?ÑØú…3FGL J1826.2-1450@0â³ÀŒLª¿ô³b ‰!ýÀ5þl3/uÀ9ÂQvYS?úȉ+bYf@º¯¾Ê@å¿ÉY$ß¿ãº/§î¿æâƒb ‰"¿éÑQa£Ê¿éh'žùTëOTHERHMBLS 5039?œUqVZþ?¤xeIøÉg?ïTuM(?¤xeIøÉg?N°wp¨ ?kÔ@§AÊP?ïøx"â#Õ?kÔ@§AÊP?Ôz¦)>')?¶þoíÃs"?å¬ë`¶ê?¶þoíÃs"?²‹a¯-?…ª…pWËI?ï‰5ÓºyD?…ª…pWËI3FGL J1828.4-1121@47	 :2+¿ÁËTŸþÀ7×ñ
õ´À9×!éBN?ö*mþ¶)@P
º?<@kÛ±í¿Ç´5§+Óm¿çN'D~ˆ¿ì½­?h˛¿ïÿkOÚ2çOTHERspp
?éñÊ#zÖö?ÆĨlƒ‰;?È8×r¤)?ÆĨlƒ‰;?ÂÑÅ?$é?É ÝRJš?ëKº°6Å?É ÝRJš?àtɂh?ºhÉãҕ­?ßlûÍÇ0?ºhÉãҕ­?Õ`üÖk
í?Á½¥YNâe?åO"Êy
?Á½¥YNâe3FGL J1828.9-2417@!Ž¡à×ÀÚ{þÀ92t]ŸîGÀ;r«G¿ñàÝ"Zrè@U<Kv?ÿÃÁá6fD¿ë9Ó>'5¿ÑÆ3îˆÎ¿áŸ‰¤X
¿Ø{Úp=CœAGNbcu1RXS J182853.8-241746?ï¦0ºÕNÀ?"¸€èÆ£ú?†sÑJ¬P?"¸€èÆ£ú?ïCg•ê?§Ž<Ѹµ‹?—Ÿ"
\B¶?§Ž<Ѹµ‹?èŒY?œ-¥?rLB?§5!w?JK?œ-¥?rL??ï÷(—V}à?T	żÙK?Q®ÑSC}?T	żÙS3FGL J1829.4+5402@T·W?íUÙ@8Ê	?Câ®À9§0IAÀ;¶½ã$þ¿ÚFØRM;@´
Öó—<?þè`·Ð¼¿àjï7/í¿à—j,Õ²¿àº-°3ÜH¿ÍÁ:Áa›AGNbll1RXS J182925.7+540255?ïû}£8¤}?Azo£0Àô?B	sns?Azo£0Àä?ïÙthpBØ?{l?o$@'?sEËÇޔl?{l?o$@"?ïgê¬{-D?5Æ(Œ7£?"ªpšW²?5Æ(Œ7¥?ïñˆšn?V¤
	ÇÛë?\ïðÊá"Ô?V¤
	ÇÛß3FGL J1829.6+4844@SNü_Ìï1@7|5_]]©À8®¥|%ëLÀ;™—û3èe?æH¢R(@eàÚv@뮟e5¿ãoÉ´i~Ÿ¿årcÎö6—¿æ 4=tU¿é¨e¾´AGNssrq3C 380?ïóÊ^ý¿ù?W.õ	8wÏ?XkB€â?W.õ	8wÕ?ïG¶kÀ'Ï?šˆŒ!ÎÝÚ?—	2‡ï¦!?šˆŒ!ÎÝÚ?ï$Ff½ÇF?"ŠpÌśz?›w3(GU?"ŠpÌśx?íѐ\9¦?ŸÑÐ.®Ü?±s2È?ŸÑÐ.®Ü3FGL J1829.7-1304@2ÚB×P´¿ó|ÔÂ^À8d"_õIÀ:&²ò0?óYœƒÙ¾Î@̼¥BÉ@öc«Kž¿ÓR|¤–LÞ¿Ù¤Ò}ö¿çw,ò§Qé¿æ‹(³OTHERspp?ºú1NPd?ž€Áhk?ï¹:ƾ?ž€Áhk?ÄžJEë?ŵ.
AÏ(?êûØmn…?ŵ.
AÏ(?ÎÇĦ1ÕM?¸`ïð:6³?èNÖsŠ¬?¸`ïð:6±?Ó}¤¬Çž?À3­Êñ4?æsÁ-©œ1?À3­Êñ43FGL J1829.8+1328@EQÅÑqw@%ŸàAׁÀ9øŽ½À;e×F£R€¿Ë×¹"Sš@
]|DÊ	y?ýîÞÀX¿è|ãN¦?Å"›-¿äž,÷b€0¿Ü£³Úž­¼AGNbllMG1 J183001+1323?ïÄ>yŸL?51P§Ò?}àÃ01Zn?51P§Ò?ï¤3÷µ+?' *ʸ?†ý3´Ó?' *ʹ?ï$€õŸÆ2?'¸Rþb0?›oáL9²?'¸Rþb0?ïeñÍ1hµ?ŠG«?"AÆYÒéP?ŠG«3FGL J1830.0-4439@uâ!€M˜9À.Oó v,­À8ÌÌ#Y¡\À;q¦½n‹?öê—é@Jô@c‰ô5–@&þûɧ¿áun°Ñˆ¿æN­q+«¿êT@([‹8¿ïÿ˜ßé#AGNbcuPMN J1830-4441?ïäCg+¬@?kT…¥ëSŒ?k¼˜ÔSÀQ?kT…¥ëS˜?ïn'²ß@°?K"6žÃÇ?'-©¤éþ?K"6žÃÇ?í]nÎâu¥?£4ÿ\Ð=?µ‰ˆìRÝ?£4ÿ\Ð=?î'r3WK*?™rä¦ v?¦èÜʋM`?™rä¦ v3FGL J1830.1+0617@B"}@XGßèˆjÀ8³È
Jk^À;	óžÈ®?ë‡	t¦x®@Éý &¼@â.Ÿ¥¢;¿Ü's'Xi¿Ý·íø@˜÷¿áÁ¼öƒ"¿æ¨GúÀ{AGNfsrqTXS 1827+062?ïø\DÍð?Pa–	ùrD?NŽï È=Å?Pa–	ùr2?ïÆV¹Ž†?¥Ó¯T?|Ôð#8½?¥Ó¯S?ï+ªS!~?"ŽÙiœ
?šŠ½Õ›Ð<?"ŽÙiœ?ïñO‰·?S(-·
$?\ý`íޔ ?S(-·
3FGL J1831.0-2714@]ä ()ÀÑkÕÎ(À9§™¼ÕÀ;1«.íSU¿ØäƒÒï@IA;3²µ@°ãŸø†¿é"çN5ö¿àÔs·þ¿ä¹¸w͎`¿á'.ohAGNbcuPMN J1831-2714?呂ɜO#?†pš•?†_͘ì7V?†pš"?î8Žs0ž?¸A¿?¬·Ìö&?¸A¿?î#í6´°U?žùÂÞ Ê?­Á,"´ú¨?žùÂÞ È?ïnŽº+ç?Š6/^•B?'.(ºƒ ?Š6/^•C3FGL J1833.5-1033@5'° F\¿ìU'?Æ$ÎÀ7Bo§WÈ>À9öáP?óæ¢̙¡@B¤ë1g@#ßâSG¿æɸµ™¿ã"ݧ)hô¿ç>EžMf¿è–¥ôEãPSRPSRPSR J1833-1034?u
#{ÉvM?ƒsøîòí?ïÕå¹m?ƒsøîòí?'×™Q™?¢eȟjøI?ïw!Aë5u?¢eȟjøI?Â.Y—ýå?·'EY³ê?ëtiš†¹?·'EY³ê?¹Ž{IU-?©¥¹{P{?ìÎ0–Õ\?©¥¹{P|3FGL J1833.6-2103@(UΞ^$yÀÒBß·7À5ü#ü^ŠÐÀ:bÁ'ïV?ÿ,ý|BØ@ ø1T‹È@†Ó8¡²¿ãæ‡Ä–µ¿çWȋA«¿çÍ~d´à¿éZïŠfö¯AGNfsrqPKS 1830-211?îæíË5Ô?¡Z3ú—?¡'#L¢¾4?¡Z3ú—
?î¸8ÎÓüæ?¶Š¨Y7?¤|sÀ1¬?¶Š¨Y6?ëa%uFµ?«>2ZU¦ó?Â{j*å+¼?«>2ZU¦ó?ïÿC±À¤P?(Xn1-?‰Çëuå£?(Xn1,ß3FGL J1833.9-0711@8‰¡_`¸§?âðÐ $ž×À7øUŽU™À9¦''ØÛ?ÍÂkä™@¡eç»eœ@ÙþÀ9ì`¿ÐÁaߙ¿äŽ8ýÍu¿¿æ†BCÇU¿ÚõâûbatOTHERspp?éÊÕÙÑ?Æþù4Iáì?ÈÔ¨˜»»ž?Æþù4Iáì?ë'€U0-?ÎN°¿µ±?Ãѵþ«?L?ÎN°¿µ±?æ?»ôH?µº&‹¿?ÓÇÀˆq?µº&‹Á?ïÃÛÒ}úô?†š©j•-I?~Á†?†š©j•-J3FGL J1834.5-0841@7HT`ªdÿÌïû_ :ÍÀ7]öÌz—vÀ9ئ²†Ði¿Û'ÝèÍx@-Ì^'Ýh@]é jƒ¬¿ÐP´ƒ)댿á¶`]Õ¿à'¿zÔ²t¿æOó]ZNOTHERsnrW 41?æÝíÁ®r?ËîqSÞÕ?ÓèD$|£?ËîqSÞÕ?瀯`ª†H?Ôɚ`½-,?Ðþ¡>ªóo?Ôɚ`½-,?åù°–f`?·,(–¿
Þ?ÔŸÜÓ3??·,(–¿
Þ?ïCÁ´²ÍB?¡æ7Ä®Z[?—‡Éi¦WÙ?¡æ7Ä®Z\3FGL J1834.6-0659@8ÍtŸå
5?àºÇà˜ÿÀ7Ã6ù'PöÀ9ˆ2芘u?"2ÛçYz@IŸæ姺@cߣê¿ë.°:Ê?ÓN˜~çf¬¿ÝV¦?oV¥¿à­èÛ÷OTHERspp?ë	uÙ»P?ÂG–äšp?ÃÚ(™Å?ÂG–äšp?ér™ŸÍä?Ñ[>îÂ8?Ê5›µ€Èm?Ñ[>îÂ8?æ¤EdbF?µyãÍ¡²å?Ò·u7;sê?µyãÍ¡²å?îX'bÞ?´¡ÔaN…–?ª}‰ßÒ7?´¡ÔaN…–3FGL J1835.4+1349@EÇç@™Å@#}1(ùÀ9ÍMüUyÀ;@'¿aª?¿Çâþx§—Å@Ä¿6@¯r_Ãßé?Õ	j¤Zp¿ë'_º6'¿à { ŠN£¿í¨Î¥êà´AGNbcuTXS 1833+137?ï%Ç>§[?Š[˜"²?ˆ¶Ž0V)A?Š[˜"²?ïFw bPx?¥‡>@4?—1óµñ?¥‡>@4?ë,çåà+?ª?h_#q?ÃL`kÐS?ª?h_#r?ï?ƒÄ.?'"-þ}äÞ?˜‡z?w?'"-þ}äÝ3FGL J1835.7-3258?øß}ž¼C=À&¾S‹'À9áB'[sÀ;¨±gìxd?øN{ÞÓ@ñæ"©r?ð2^צÅ|¿Ñ×Öì
¶¿Ý•»~ã¿éœolŸe‹¿ïÿ\×qk}OTHERglcNGC 6652?p¹Ø´E"¡?vE?êH£0?ïތN—uº?vE?êH£0?iùõ²m?†œkX#'ï?ïæá
Mì?†œkX#'ï?¬sý

æ?¡X*LÓo?î8ÎÀ/_"?¡X*LÓo?‹óU'ÎQÔ?€¹8M¶¢ê?ï2©´Æ¸?€¹8M¶¢ê3FGL J1836.2+5925@V8tÿñ½G@8ÿ'¿°"˜À5<³»ƒÏ-À:YÌÅ@'@ oa6Ò@Րà?õ:€nû5k¿¿NšlÓ=¿Ûʬ"y
¿æ*Ü#,¿î¨Hî}ÃóPSRPSRLAT PSR J1836+5925?.Àù?Cה?$Wª¬ël§?ïþðlÃ?$Wª¬ël§?fÃÒ>ÓP8?};€Åã±Á?ïé<-Á,¯?};€Åã±Á?£Öì|¦?ž!>ÿ?î'8?õž?ž!?>'wؤkÊ>œYî?ïÿÿ·Š ž>œYí3FGL J1836.3+3137@N/sßË­@0É'àÙìÀ9_Ñöy}À;t.QZ¿³ˆœ•N;@Upõ¶@ÅxÀ01K¿è"¼R"®ù¿á†¢®7­¹¿æοë+¿äÅ4
^ôAGNbllRX J1836.2+3136?ïîŽ;?‰—Ø	W¸?aqÄåøåú?‰—Ø	Wµ?ïÔ²½r'œ?~KµüX¨?u¦¡Fì1?~KµüX¨?ï/&ð2Å?'M–ÑSÄ{?š!ù½§Z?'M–ÑSÄ|?ïÜI¤ÅÑ?gE¯U¹Î?qÛ-q?gE¯U¹Ê3FGL J1836.5-0655e@9áj("?Ád]?Ô´ÖÀ6ñÖ³Ö\À9K~Íey¿õ«µPy@l«…Th7?ÿv
`:Ó;?ïŸíp±C¿ã2dkºc>¿ä5»wà¿ÐÞC\vyOTHERPWNHESS J1837-069?í«›« ã?º…è}3®?·Z£"¢øã?º…è}3®?íZìZèí?Ǩ¿È—ò?µ(Ÿm(¸ ?Ǩ¿È—ñ?çyP·AÐ?µ‡½ZMÎ<?ÑÓ
^'|_?µ‡½ZMÎ=?ïûÛ«…Ž[?YŠ1àLÞ?@'Qéƕ{?YŠ1àLÞ3FGL J1837.9-0607@9ò€Æ^?ÈÎ_âáÀ7à~SÂõ³À9‡¨ÖM?óêy¶O\ß@ô.·x|¾@"BÀCý[¿ìNùõœF¿×Tj*Kâ¿çfjÆÙ~ó¿çYG·y©dPSRPSRPSR J1837-0604?ˆiފÍÖv?—PՒ2?ïžX…ÔȦ?—PՒ2?È¡ Že[w?Ê=nÍ/?é×·Üf©"?Ê=nÍ/?ƕ˜`§`Ç?·Ãïúoé?êZ™çÖ'Î?·Ãïúoé?ÐæDþ˜ ½?Á'/Pc­?çŒÝ€³¯¡?Á'/Pc®3FGL J1838.5-6006@tõýç!À5½v Í|À:$Âî&¹¨À;¨¶urrä?íuúÅn@2E³"k?ý´Ü€žöÑ¿â6wM‹Æ¿Ô€[j3ûZ¿Ø3Tq­}¿â€åC!ÆAGNbcuSUMSS J183806-600033?ïSmÎAÀ5?šë""L<?•'F7Çù~?šë""L<?îo‰ûð^×?´±¦R?©`@ú"?´±¦R?îØ
Èé¤?¡}âÄu9?®rSqeË?¡}âÄu7?éUÈZéÆò?²Áàς¿ø?ʨޔXä7?²Áàς¿ø3FGL J1838.8+4802@S<b?û˜'@5ÔC@ÇplÀ8öïÕ'À;BL¨O??ԟ|EºŽ@¤%D24?üåâDhæ¿ãEÑøGq¿ØýÁ†óyµ¿×bÝÈë0¿ÖŽ¥nRÝ·AGNbllGB6 J1838+4802?ïü+œº"¤?:ÉÀÝGˆ?>£+Zå@?:ÉÀÝGª?ïËãÚ΁á?'ŸWò?z˜¿n?'ŸWò?ïÄÄI³÷Q? áR?}Û&XD? áY?ï¢ÍÐó(?xH|"œË{?‡L‹ü6<?xH|"œËz3FGL J1838.9-0537@:€o_3l>?Êxßl>À6ŽãðÕÀ'À9>áÃÔև@¦`Ž@
Ì]ÓG?ÿ}³Áä¿Ò˜b0Œ¿åÈmÈì~ª¿ã…j²SŽ¿ìІ^1PSRPSRLAT PSR J1838-0537?PÆNi'ã³?TÕρåÊ?ï÷œØË6?TÕρåÊ?%˜IYU1T?@Ý×	?ïþ¦{jj¬?@Ý×	?¬¶}ˆg"f?¤û3-4Ú?î4˜'y†¹?¤û3-4Ü?4•¦Å‡?1'®~Ú?ïýnM_«(?1'®~Ú3FGL J1840.1-0412@;å`Ÿ}i?â£t?ܨ§À7«À_AÀ9Íúꉯ?õ{*ˆ"¹‹@?­le@Sõ?ݐ"¿âgrÕàqÅ¿èƒÝRu¿æß0$˜;¿ë"Ï"gˆûOTHERspp?X$P©À×?‡לox¹?ïóøm׫?‡לoxº?UÔ1?s;êj £è?ïõçwù¸?s;êj £è?¾êué Iå?¯ý˜/ð!?ì"±BÛöÃ?¯ý˜/ð!?"–Ó6ÿOÕ?z!ڒ¶6?ï­¤³$Á?z!ڒ¶63FGL J1840.9-0532e@:ËÂ@ÐO¿Ékd'õµÀ6¦rKPÀ9FS£C^?†è×sñ@ÙÀ»¡V?ü㪟PgÌ?ÖzwéDR¿½EÁ\\¿ÜàÝÓNq¿ßϓ¼
êOTHERPWNHESS J1841-055?îâWâ½I5?¬­™^iõí?¡ÚÔ+lº?¬­™^iõí?éäÙ!¤?ёµŠáIÌ?Èl›{³éo?ёµŠáIÌ?ë•''C›?¯ß'©´¹¥?Í©»bñ–?¯ß'©´¹¦?ï"A¯¸?™/×e¯æ¨?Šþûo"ù?™/×e¯æ©3FGL J1841.2+2910@M8"€,á
@-É0ŸÚü:À9ØÏL
ÑÀ;`,ÖøŸ¹¿íό‰Š@
Ž¨'ƒ?ùóÀ+©§¿ê2þÄZ|<¿áÖ©Ôò'‹¿ãijù—03?×ûîwUnAGNbcuMG3 J184126+2910?ïî;È8ä6?cV-ólöÈ?aÄ7ÇÊ6?cV-ólöÍ?ïÜÓ䢄Ž?{y¶Ô?q–
®½¹©?{y¶Ô?ï/Æá÷Ë?'À
ïÃ=
?š#߁_?'À
ïÃ=
?ïþaç*?/·µð¾i?)áÿÍp_?/·µð¾V3FGL J1841.7+3218@N¾'?ßéà@/úÖ 2¥oÀ9J±ÓLBÏÀ;i»Þh¿ðôFn#t#@¿nëE3@v>ËLo?ÑÑ£=S¿è¿èiÜ̳¿Ý9"ûƒƒ¿ÈYÀÛÒÏAGNbllRX J1841.7+3218?ïýÒ)
Ø?2¾f­ë?1of·'Fd?2¾f­í?ïâ&+]½×?x*ºÃÁÆò?mÙÔ¢B(•?x*ºÃÁÆò?f‡ðC?‰ü€]·@?æ^ï>?‰ü€]·B?ïþÇG–1?%€¯ißZz?#Û†œþH?%€¯ißZe3FGL J1842.3-5841@u?«ºÀ5Ë{_ò®ßÀ9È*"yÀ;~¾|§ñ?ÒCP@y¿@
»?ÏM?û ÷ÿ«q]?îÓ
;°bç¿ãÔÃRis%¿Æ[h…`¿Ý
7+÷eäAGNbcu1RXS J184230.6-584202?ïúß@<YÜ?HbCzFþŠ?D'ÿ˜¯?HbCzFþŠ?ïÓsÔhÕ?sìÒ?vF˹?sìÓ?ï§	zj6ø?ƒº;ŒÑ?†=¡erAœ?ƒº;ŒÒ?ïÖÐ.}$	?jšä-@ê†?t—èÁmûm?jšä-@ê'3FGL J1842.8+6810@X£Óßæ…@9ÕiÀú)À:-¼±Ì–FÀ;¬à‹Ær@¿ðiö¾¸¸@wd/¥µ@jrà_Ý¿ãgŒ"S¿é´µÜ<ε¿ãNtžîî¿âì?œ€²KAGNfsrqS4 1842+68?ïÿìÂûAL>äMâPÇéc>ã=¾²Jl>äMâPÇâû?ïàv̦?zœc?o‰3æîYP?zœc?ïïëk|?f&}›&B?`ü甃'?f&}›&@?ïÿ+d ?xv±o?ó{ìˆ?xv±3FGL J1843.6-1114@6
€_5ð}À,ß?ëþ@À8¥
¿cíÀ:š`' ×?ò— rç(C@DO‰€ï@ϔÀkëa¿áyÁùCñ¿êi¢'¿ìþ]YÙe¿ïÿzö…ÍPSRPSRPSR J1843-1113?ÕgTÖXò?Ïbˀu?åLU"Ó†¹?Ïbˀu?–²Ökúë:?¶z~×nu?ïJiL (§?¶z~×nu?Ù܃ŠÑ¯l?·+:Œ:H°?ã¾:—(K?·+:Œ:H°?>8ûN?€îÓ§òä ?ïƒÿ¦?€îÓ§òä 3FGL J1844.1+5709@U­aÿÏX˜@7z—¿¤ÆÀ9»J>³‡À;ÃhEc·_?Â%¿Í_ïª@Ó¤'UÛ@\ 'F¿¿áê£Åê0¿ã3xV¿ãµÝúòz¿ïýÎ xµ7AGNbllTXS 1843+571?îAD/ž–?°éoº3`?«ë½–®?°éoº3`?ìæ¥Éo¬ã?·…s• ˆÔ?¸ÊÑ´'˜ñ?·…s• ˆÔ?ëær"~ã?°'e°L€?Àf7Åîw?°'e°L€?ì½È=Ýj±?¦¿wul[7?º¾ªz?¦¿wul[73FGL J1844.3+1547@G&	_ûZ@!RaՈ]À8ºë"ùÀ;µ}û®b?èqP¾ù@'L(!²,@9v7]d¿Ùnÿmš‰¿×¦on*ˆ¿â›®rÕÆ­¿â W·³\AGNbcuNVSS J184425+154646?î A12?§pKÎ1–?¥þ[ìïÌÓ?§pKÎ1–?êàvYë¾?ɈÊé7ò?Ä~&›˜Q?ɈÊé7ò?í0.O <?¤ø$dàè?¶Ž†þ"?¤ø$dàç?ä'8¥q¸?´v£4=À?×±Øµ?´v£4=¿3FGL J1846.3+0919@DX[_¢'@j!€-aãÀ8l|ÚF2À;$î?
\@üɦ&Ž@Mn=p3?îe@×\?¡þöÉ(0(¿³',²Ä¢¿á±Sißl¸¿ì…0-Å5)PSRPSRLAT PSR J1846+0919?{Ï!fE¯?€	"ØE–??ïÈa½3uþ?€	"ØE–@?eæÁ""_?y˒9i.?ïê>lún?y˒9i.?"""Ï1@â?–>å÷Ú6?ï^ëنuù?–>å÷Ú6?i[5év&!?]8¸
£t?ïæ¤Ê‰Û?]8¸
£t3FGL J1848.1-4230@vó¾ýÀ1cŸVqýÀ:)+rt'À;ŠS².»Õ?àAšƒhC¥@
n¦9R?ÿ8ÿ€SLƒ?ï2_zÜ6š¿ã¡[Dý¾¿Ùd¦ÙÚ8¿åb©a§~£AGNbcuPMN J1848-4230?ïÚ&ÿuvõ?}¨ÙS
~Á?rì€ED"Å?}¨ÙS
~Â?îúøô?°'Ǘ"5? P¾ï@©?°'Ǘ"5?ïê†ýU?˜ùñ1?ž° U2?˜ùñ5?íÏíW5?£í¤Z
Š¼?·a€—}F]?£í¤Z
Š¼3FGL J1848.4+3216@Oˆ M@-[ç^jÀ8&	Ñ:×À:_ÙuQ»´À
˜wDŽ¥@p'º}ý@JÇ?Åí¿éªî
¾à¿Ü&âå4o¿æ´Ô¹]⽿äVžÙZµêAGNFSRQB2 1846+32A?ï½F÷F0Ê?Š6ysÎÄ?€®B.s͔?Š6ysÎÃ?ïå§åµÑk?z¡¦h…Û»?jXJ.•¦?z¡¦h…Û¼?ì}Å(‹ª?©zÔ¸Ó¾ö?¼מ»¢°?©zÔ¸Ó¾ö?ïÿÿùž±C>bmžshªý>I…:õ¸î>bmžse£«3FGL J1848.9+4247@RÁð`P@2{_L–²À:i»dgÀ;¹ZúøYC?èéQ×|î@ G"g{d?úV¾|'¿îÃò¯Ø¿ÇJÀ©º	b¿éµ¶¯]Ò?åwÈ/üiAGNbllRGB J1848+427?ï~YHï¼?'áÁÍM?4ÖîB3?'áÁÍM?í¯aO? n'?°?‡Þ""'¬Œ? n'?°?ìLOn¨Í?¬CzR'›?½"Š¼™?¬CzR'›?î˜ìlja?©ÁðKÌÿÙ?¦q3Ž7ià?©ÁðKÌÿÙ3FGL J1849.2+6705@X_[íöé@9
` ÒŸÀ7¼0íޕLÀ;)ÆΆ
q?øÖ)vò@8t1Bî@ðwy‰-ç¿Þã)ß]¯¿ä Ì=R=\¿ä]ŽGoÄù¿æàS*°"íAGNFSRQS4 1849+67?ïý—ÜSV€?6ÝUò%*?3AeKü8?6ÝUò%)þ?ïÝÀœIaŠ?~1¥Ø·ÿ?q±ÛO;?~1¥Ø¸?îÐnt†ÏO?˜;Gm
?¢ù·"1?˜;Gm
?ïÿäÆÿ¾>óa
ÈPƒ>ë9ð@«í>óa
ÈN3FGL J1849.3-1645@1³q¿_üÀÀmœ@ÔÀ9Ö®8HÀ;=Øwûº ?çºõ¬¿ç@
~ Lf?ù°ŠŸ*Ó?åUc¬En¿ï÷Š9™­?ïÿ}'Gÿ"¿Ú	ÞxúE_AGNbcu1RXS J184919.7-164726?ïê
º	?nPO•$ï?eòèEâö.?nPO•$í?ï'UÅ?°‰Åä :?œû¿õG{?°‰Åä :?îßå{‡?—žòGŠ?¢¨GÞß?—žòGŠ?ï͎Ìì?˜ïr»Ø?y8™üòŠ?˜ïr»Ø3FGL J1849.4-0057@?Úý¿³ß–?TÜà‹À7½ð÷3©À9¾Ç¦^Û?ø»òː7@y'W'c?ù'cð?m©?ï	Bi1¿Íƒ'[·¶»¿ãµ3S£K¿â¯ò6á"OTHERsnr3C 391?½®QŽy°'?¿õÀ©?ìJ5Î0Éî?¿õÀ¨?¥OÍ+7?¹4{į
Ç?î¯K-LŽ?¹4{į
Ç?َoLw¿"?¸ˆ²ÅŒO_?ã8ÈYÄ 6?¸ˆ²ÅŒO_?À¤Ú{ý6í?´Ä«ŒSZ?ëÖÉa²E?´Ä«ŒSZ3FGL J1849.4-4312@vx@À1Ú3çüÔÀ9C΋é®À;UÏ2e®?꬝ØB¢@ê#3
ïG@"›€y
¿Ñ¨õRäÄ¿á9£ª¥}¿áҜH[ʒ¿æ—þ7d+ŠAGNbllPMN J1849-4314?ïÍösV?zI ¿YPv?yüsÆT‹?zI ¿YPw?î¥t>®?¬ËO¶;éÈ?¥¨¼NÕ?¬ËO¶;éÈ?î)S÷Né?¡…K9+E(?­ozÀ‹b?¡…K9+E(?ì;Sí#ù?›éôŽ	g?¿%`–à:?›éôŽ	f3FGL J1849.5+2751@LøÌ?ß @)a ˆ5ÄÀ9µ§íÀ;~¬ 7?ñ5†oE],@ãîƒ*í?@¨8ßðk
?Á—'ӝeE¿äši¿ê!Û®"N¿ë.¿±qAGNbllMG2 J184929+2748?¦å6û­k?°q²ù ÎØ?ž E)?°q²ù ÎØ?Ý͙VÅ-?Ñ-ǐ0¶?á38Tj?Ñ-ǐ0·?ÎÊlf×n?¸º£?èMydæJ$?¸º£?ɧ[öa,ë?«><¶~/a?é–)g´Å?«><¶~/`3FGL J1852.4+4856@S¦ó?þÑ@3õà_PÈÀ8†oÔ¤1£À;Œ.î¿¿ë$ồ¶Î@˜qB7ˆ@|yÿËQÍ¿â?J«k‡¿å¯uˆ8¿ã‡fýŸ¿á¤mÇr‰¤AGNfsrqS4 1851+48?ïÿÜLG‡>ðí¶\ª<¶>ñÙÜ<u÷Ó>ðí¶\ª@&?ïàÆîDE?xµ&îôä?o9ó»ºp?xµ&îôå?ï؟åhQ?t•wŒšåw?s°
K÷Wq?t•wŒšåy?ïÿøA_[»>ÔÂÙÊzò¹>Îú''þ>ÔÂÙÊz÷š3FGL J1853.2+0006@@€ŸÍA¿Ö!Ÿ¯T¹À7¨R$AÀ9í
ÒÁÙT?þ™ ÍÕá@56B²,@6L,ÔIn¿ápòÁ~%¿çr(+mA!¿êˆyê/g¿ã­_cŠ5pPSRpsrPSR J1853-0004?–ÊU©ì!?®Ç&l\ñ>?ïKñ­R°Ÿ?®Ç&l\ñ>?‰ƒ<Ý.è…?®ËÔòæë¸?ï™ó‹D^?®ËÔòæë¸?ÐÖI}Óã?·5ÀÖ¤HÙ?ç"ÛA}
?·5ÀÖ¤HÙ?"‰‰à€?‹‡
kڍ¹?ïc³³ûý?‹‡
kڍ¹3FGL J1855.1-6008@tþí )À7½F@V1eÀ:Îç·3ÞTÀ;úŒ3‰M?çv1Npj:@›Â[YÂê?ý'(º3?îÀšdoÁ¿ÔÜ	
•°+¿ÂÜú.&Pn¿ß
ZO4y7AGNbcuPMN J1854-6009?ïÆÎZ-?‰¹Dwû°?|ðýÒèø?‰¹Dwû°?ï{†ìîø?žœ½äo©¹?"b=`à?žœ½äo©¸?î"ôCÿìl?›Q¹T‡È?¦°»À9J?›Q¹T‡Ë?ìÝ#©íËr?¬-äþày?¹Ⱁ¤l?¬-äþày3FGL J1855.1-2243@)½«ÓÚÞÀ%ÙHßlâÀ:IR}ÔAÀ;ˆÙÔLg?ðÖ{<6g@.ÝTYs?ý"ÔÁ7î.¿áøK€±ì!?é€à¶cª¿»-""Ñ¿ä¥wžG(^OTHERglcNGC 6717?îo&}§Ý[?®'´¤ÔÝ?©
˜%'*F?®'´¤ÔÜ?ë|ÚÏJòÌ?È.¾'Wo"?Â"ÂÔ4Ð?È.¾'Wo"?ëäAÎö<?¬S°þç›m?ÀnøñÄ'
?¬S°þç›m?ë¹}Ú	œ5?¶*Ûª;x?Á—ُ-?¶*Ûª;x3FGL J1855.9+0121e@AS°
kù¿ØÙ"`}ZÀ5XôÀ0ÝÀ92ÛŸ'@¬	íI@Ö|O[ÝÌ?üNoVÏðn¿Á~õÔX¿â*ªcy¿æ;êý9|#¿ëvO²ÅºŠOTHERSNRW44?ÅD{ŸHyü?Îð—ò…Ä?ê®á-á?Îð—ò…Ä?4<g4IFç?Z•Ú!Ç4?ïýxsv×?Z•Ú!Ç4?ÂÇð-à?Äîýäqu
?ëNô‡û??Äîýäqu
?M]7"LI?N\]Ç7¬A?ïø¨²7zm?N\]Ç7¬A3FGL J1858.2-2215@+5}¡ŽÝÀ&»Ú@RÖgÀ9'Τ=aŠÀ;‹½÷FóÚ?ý…'MJ@C±Û"Ì?ð³!Ø?ËwúzQ¿ÂŽúPµò¿ç·f'¸¿í˖ìÁôPSRPSRPSR J1858-2216?TH@™l‹ô?S³m9·I;?ïõÛß³I»?S³m9·I:?y»:­ŸÖ?_NDÏ.˜?ï̉͊¤¿?_NDÏ.™?‹Ó¨øÌÛ$?ºƒ˜í6?\̓?ºƒ˜í8? £ß!¹/?‹µ¹ŒG²?îÿõÂ
än?‹µ¹ŒG²3FGL J1858.4-2509@%ׄABÀoÀ)8!4x®À8Ý-?~À;7é;˜\ƒ?ðÓDá"@¸vb\ìj@Lú¿¤ED¿Ès˜•¯÷v¿èÇON6¿àYÖú¼ãå¿ï	Aš:eAGNbcuPMN J1858-2511?ï¯!ç5Ê?}öxæ@"?"7†2zl?}öxæ@?îZ~'Åá?´ È/>l?ª^HÓ¢?´ È/>l?镉-K2?¯oo=Ž?É«±ÛJÓ4?¯oo=Ž?ìCMÙ'?£	M±š"\?»}å'7ƒy?£	M±š"[3FGL J1902.0-5107@u™ûoÀ6c
?ƒ£ŽÀ8}ík¨ÆÀ;{,Ü×ÜË?ýR=›¥@T˜"#@Ä Wì%¿Ð!°¡?w²¿äPàɪ·¿åÇh>Â*¿î9uýˆ+ˆPSRPSRPSR J1902-5105?q럔fÚm?vÀ˜"˳?ïÜ(À×2K?vÀ˜"Ë´?"\Fžî?¤ÌZñê?ïe%Ï[
?¤ÌZñê?±¸.q«Ó?¢Á¡õØ?í߈ú1ʆ?¢Á¡õ×?'Ò´ÞgžL?‹›½®r9K?ïqjYÃ
?‹›½®r9K3FGL J1902.9-6745@t} FÇeÀ:
%@+i:À9~s£eË6À;¾ç!â¨×?à8u_ÜA@Ü¢­¿ke@ÄÛ Ú+¿ãzƒC8[^¿ë:Û}ó)¿å9ËP©nV¿âógŽ¸ÅAGNfsrqPMN J1903-6749?ïö'®¬e?'õp®ëy?RÜ¢§5ËÌ?'õp®ëy?ïߖ0€v?zѬMXW?p4Àg¿Ås?zѬMXZ?ïv²#É3¬?Þš=Û?')»†ÙŠd?Þš=Ù?ïñ[Imª?Rñ?wÅÚ£?]Im$¯?Rñ?wÅÚ½3FGL J1903.2+5541@U~¤?åÉ@4‡ŸŸm1À7ÿ®õKqÀ:Ë>³™õà?ôźߺeA@¡Æ¹¸H?÷_~«+½H¿ÙžRÌ£¿ÕŸ=X® ¿Ú´!!sÿ¿á\äÓºãÒAGNbllTXS 1902+556?ïî°½¢6?j˜WËDRð?aOïB]ÊL?j˜WËDRí?ì9X–(ì`?Â1X¶^œ?¾5;N¸œÿ?Â1X¶^œ?íJy©†›ó?§™ÔĤà?µ¬2³Ë h?§™ÔĤà?ãýï«?·ëGÅ©Ü;?Ø!ãâ©â?·ëGÅ©Ü;3FGL J1903.6-7052@tEõŸôýmÀ:'ë ÍjÀ9"=çÂÀ;¤®Zþ‰?å8æg—Wº@¤ý)+@‰mèþ‡¿çxû@Ÿú©¿Þ*Y©ÙF¿å50ûdS«¿í˜™ç2«PSRPSRPSR J1903-7051?Ó<»wvñö?ÉfÓýÅ5?æa¢DD‡?ÉfÓýÅ5?Ûº…Ãv^?ÑOÌz­?⢽DÑ?ÑOÌz­?á°ZÖß²?»kÜÜg4•?ܟïJR@?»kÜÜg4—?ÝââÄË*?»|…]‰Œø?ṝšk?»|…]‰Œø3FGL J1904.5+3627@PÕlÿݛQ@*˜Ý ·0À:HŒŠ½À;»©°h8?)z?¾´?@
*)Ö=8ñ@ÉXŸÿ9\¿ïÿó´ÿH?ïþIãñ#¿âޔ`}Kä¿ÛýëJDAGNbcuMG2 J190411+3627?ïõ}4±è?Uxª°‰?U–Ø1?Uxª°?ïSkð½p"? Sw¶[¢¿?•'èQûÊ? Sw¶[¢À?ï¤j|¤a?µ"Œ1.?†å`Öügz?µ"Œ1.?î2n5M* ?¦´ìu6?¬Ù«-]þ?¦´ìu63FGL J1907.9+0602@DúÀ%¿ìÔT@(4À5ݜ©'žÀ9êXR§lÁ@.[ê¡õ@ÿI@eË·@$̦·9¿Û²oË·Es¿ãfCo°+¿å‰¥ì@ãþ¿ìëè%óôPSRPSRLAT PSR J1907+0602?[¾'"'‹™?gÊ¢þþrt?ïò ·=ì;?gÊ¢þþrt?̓`gÞ?4ˆ¨q]¶?ïÿ!"äÿT?4ˆ¨q]¶?¡‰u¼±Äa?¢' «é?îçh¤4ã»?¢' «é?+üú'ò´y?,¼‰ˆt?ïþ@0VàÔ?,¼‰ˆt3FGL J1908.8-0130@@ÇûÆnåÀ9±êFÀ9ªð]ˍ2À;²g†÷Öf?øçj@
ÌiûqOù¿ëyÖ1iH]¿ïqªôy¨Ò?íåO[¿æöË,¨nb¿í™\ZHö¿AGNbcuNVSS J190836-012642?#¶› ¼Â?²%nôŒuÃ?ï‹q%'}?²%nôŒuÂ?u°iÁ(Œ"?«T0ÅÑ:ù?ïԟ,}®ç?«T0ÅÑ:ù?ÀÆÎ9·x¤?¬qÿ|u?ëÎLq'!×?¬qÿ|t?|šzr1¦ž?"…X7
¨y?ïÆËœ²?"…X7
¨y3FGL J1910.7-6000@u"§e4À9žÚà‹ÆrÀ9ÚïÅYbÀ;Æ{…²\?ô£D",î@ÄáÖõÈ@š½ …«¿ä»Û®ã¿Ù·°ÛÕ~L¿çæ"gÞá¿í»ûÄ1OTHERglcNGC 6752?‰ÄtŽ¨f?Ž÷ùBK‹?ï›ôî-Å^?Ž÷ùBK‹?'úAqT?ÂÙ5w;?ë[A¯£«?ÂÙ5w;?ɊRúS?á?±S—\BÄ ?ékAk0?±S—\BÄ ?»Øøi®­€?¤Üª+õû?ì"àòÊ*P?¤Üª+õû3FGL J1910.8+2855@N{À?ö@!ƵÜê&À:8ðvö£À;€d%C†h?é{noc)	@
~†ܖ?÷jŸÁ%ú¿çZÝ÷lˆ"?ïÿª,cä¿Ùd¸&'B¿²¸oÕrZ2AGNbcu1RXS J191053.2+285622?ïÝÞK?q§b
S¢›?qwòž0Úy?q§b
S¢™?ïW8«Q9?«D¥ßïñ;?•üj•Øã?«D¥ßïñ;?îöócb‹±?•Nù°šs? ÉÉ×Dï?•Nù°šr?íP©fý2ï?¬Z˜õ½fš?µz´Èh'?¬Z˜õ½f™3FGL J1910.9+0906@E ßÔŽ¿ÃäH~ôÒ¥À6k3æÉÎÀ9–M$v?ú´'ÇÅ&@¡NÇѐ?ÿk"Æ(˜Ð¿ßc%  ¿ä\áýál¿àUf.2Br¿æ´7À
DŽOTHERsnrW 49B?« ä'Ž
ú?®ˆ•â,¯a?îEñ¶×!?®ˆ•â,¯`?`,‹|0v?yPÀâ?ïïÓ~tƒÐ?yPÀâ?×Ʊ՗• ?¹‹ãz(?ä§45/?¹‹ãz(?¢¦*rÜ7c?˜¢"ÛÆ¢½?î՝XÒ<‰?˜¢"ÛÆ¢¾3FGL J1911.2-2006@0â
_ÕR­À*sç_JHÀ7ºÚ4"\À;Êʔ
i?óusºaæ$@´›Ü¿ß@E¸7~¿ä_Œ+Hk¿å¯rÎ"`¿æԃâu¿ê]8ÉÛxAGNfsrqPKS B1908-201?ïÂð×?Ùí]0vS?~‡ø"{ð"?Ùí]0vQ?ï˗â¨k?"5ÇÜÃ.¼?z4«øJ¥?"5ÇÜÃ.»?í_±ˆ¸VÍ?¢^w@
±?µsº=I˜?¢^w@
±?ïøӅ!®R?G×¼•‰êt?L±ëyF·Í?G×¼•‰êz3FGL J1911.4-1908@1ÑŸ>õÀ)½ôafLeÀ9j+Q½aöÀ;6dE#ö?£7.aߐk@"î´þúÇ?üQ¦áUÅÚ?ïµF2`Ǹ¿Úá–|y<¿ÒèÛµ ®¿ÖŠÛÞ$AGNbcuPMN J1911-1908?ïò²Ï=ÑÛ?Z]ä¯H^Q?Zša"\J«?Z]ä¯H^S?ïȈÿ˜º?†XånD·?{»÷3£š?†XånD·?ïŠÜòL¶?"²þäǵs?HÃlùR}?"²þäǵs?ïßz2!ý?cÓ¸Ž;ÁÈ?pBæïxÒ?cÓ¸Ž;ÁÑ3FGL J1912.0-0804@<	I`œ"
À }ÖOÀ9~ø&²òÀ;Œ#QA¿É¬v|DZ@Z¼#jR@\"Ý¿ëÂÏÏÐQ+¿ÔÎ)¦cú¿ßrצQ'¿éú–«õßAGNbcuPMN J1912-0804?ï‹!ÃF4q?"vÏN±Š?7.rã´?"vÏN±‹?ïBñu<øF?§)ê1LÒu?—¡ÑX`÷e?§)ê1LÒu?ìd¹ûҐ?¨ om$^?¼Ú7Ø!k~?¨ om$^?ïâöó•"$?fœ8
1û<?m	jÝÛê?fœ8
1û:3FGL J1912.6-1223@8+OP À$‰®ÁIÀ8Ú7æ÷~À;!•ÄøÿÓë!Ùf¹@¹ø`Nt@ïÜÀŠÊ¿çƒÌZáøÙ¿æÃqù[dï¿ä8,ŸÎÅ¿âñn±}UAGNbcuTXS 1909-124?ïÿ!jÕo? *h 4°	?Ò½eQïZ? *h 4°?ïo a(«? É>oÝ?'ý³ÚêÎ? É>oÜ?ï¹ðœÿ'?".Nç(&?¹ƒØÀW?".Nç(&?ïóŸÿŸÃ?Pz4ÿ™»?XÀàÀxy?Pz4ÿ™¬3FGL J1912.9-8008@s <€"ÞÀ;c¿ÂùÀ8²gˆ¥UÀ;CE?¥1}?÷õýR{¢ä@ÿÿL%óZ@il(¶X¿àøm"—ø¿âøëÒݙ4¿æ€;WM¿êŸ½¨ %AGNfsrqPKS 1903-80?ïƒ.»µ…?ŽLUlwm²??4Qžì?ŽLUlwm±?ïޜ"-yd?v˅nòë?p±µéCMŽ?v˅nòè?êQXÐ$?¯OÞgôz?ƺœ¿‹£n?¯OÞgô{?ェŒFú
?x	ŪI‡€?€•\îA|É?x	ŪI‡~3FGL J1913.0+0910@EÇwàmò¿â:þ Œ=À7éç3ö¨À9ʜcxu]?ý"T¦uu"@
Eq•n'®?ýiš¨¸E?ïÿf#dLõ¿àñfœí1¿éíM¦¯ŠO¿înÂÛ(ÒPSRPSRPSR J1913+0904P?\ÓÐ$?'M¯Ò'?ïñ–~ž}·?'M¯Ò'?3{û´ž?IOe§ÆU?ïýž€‰k?IOe§ÆU?¤#Œgé€?£òš­Î?î½Ç9gþ?£òš­Ð?{ÖtT_‰²?uS¨ŒlÊõ?ïÈSW@í?uS¨ŒlÊô3FGL J1913.5-3631?óA« §UÀ3å*?nªÙÀ9·ä$gÀ;qBÖ>f?؟ºoýéÐ@lôÂ4B}@K^ tT;¿ØÎÖ1¥i‡¿åNGÉö·5¿ãaà·);Q¿ãÜQFAGNbcuPMN J1913-3630?ïÿ*ڜ's?! pmNЎ?¤¬o±ž*?! pmNÐ,?ï֟¾Rê­?úÊ[!Gï?t° ֊©¶?úÊ[!Gï?ï˜}"Xl?‰¾íaAÄ?‰à›)þ¤—?‰¾íaAÃ?ïþ­Y¼ýq? š|z'{g?%*d0(ïp? š|z'{y3FGL J1913.9+4441@Rö+`Ø@-÷™ÿðæˆÀ9úâénÄÀ;ª
ájÃ?Ü<<
Lo@F¯ÀÍe#?ýužèó¿å07õËÛ¿ÔúòàæN¿ÔÔߜC~@¿Óž£:†§AGNbcu1RXS J191401.9+443849?ïï¢àøm?[Ÿã<'˜?`]'ü?[Ÿã<'Š?­Oeþ?—g*2o,í?Ó"¬&€µ?—g*2o,í?ï—"@"?'³•†éj?Š<w{¯Û6?'³•†éj?턉2èXµ?¡€i'üùU?³Û¶h½:W?¡€i'üùU3FGL J1915.9+1112@FÙIàâi¿Ñ._ܒÀ7ý:8
2‰À:;i…Õ—w?üÐ=‡Êå@‡žT"Vå@6ßïiYá¿á­å_—¿æÄ
¡C²¿è>ÓåÅ¿ïþ—ëC°YOTHERspp?|Å©Ô6a?†"úò8ë ?ïÆt¬W"Ä?†"úò8ë ?8¸ø%s›˜?T¼äé¦m'?ïüèàûQŒ?T¼äé¦m'?¿b.¨R?¯1X:ï¿7?ì¬Z?Šö?¯1X:ï¿7?zó܈æÚV?lÖ"Po<?ïÊFî2L?lÖ"Po<3FGL J1917.7-1921@2<‡`±ñÀ,§Úáb†À8'Yáó¥À:Îÿ€¾?ãÊåÁæ?@'"T±I?ýòÓÿñè:¿É¨còÿ͑¿ÜøÉkI¥¿ÝF*ú¿ÚÙ©Ê>R AGNbll1H 1914-194?ïë¡»¤°í?c§…ˆ+W?d^D[O¼?c§…ˆ+X?ïŽÓæ$œ©?•—ÖÄ¿:"?ŒKvØÕ×?•—ÖÄ¿:"?ï+†åYe?•»±°ú?š<ƒTÓe?•»±°ù?îöÈÐØk?'•Pã÷Qí? "rÿây??'•Pã÷Qî3FGL J1918.0+3750@Qqb¿è¸¼@&äÔßÀÅXÀ:jå€!ùOÀ;ÅÃqÚ7ï¿ûŠ­ Œ§ï@j£¼2K@‰_²?¿å_Á¤$·ð¿ãÞOªüÝ%¿Ø¡=6÷ì¿ã«ìE@¯{AGNbcu1RXS J191810.2+375315?ïþÕyS9)?#ËÐpÈöi?"¨jÌm†2?#ËÐpÈö€?ïÙD3	0µ?~ª]v×?s]æ{g¥´?~ª]vÕ?ï²Õ8ƒYà?ҕðŠÅ&?ƒJ±ß)ˆ?ҕðŠÅ#?ïýî/¶h?5Þ\_ Ï?0&'L®?5Þ\_ ö3FGL J1918.2-4110@vL» 1ίÀ6=QÀ¼ôÀ8ŽÄ¾áQ¿À;E%£þw?ù®:m$¡@Àn&nª?òÕ5 É#J¿à;Y2~àä¿Èì0g"/¿ÙÖwø×d"¿äü/Ö(ãpAGNbllPMN J1918-4111?èT»Ÿz?ÈÑ؄éi?Ϛ­ƒ²?ÈÑ؄éi?Øüö9þ¡à?Ò¡€{ú?いã¯?Ò¡€{ú?åø
ÍuQ?¶v®'ãFâ?ÔêeÇ^?¶v®'ãFã?ÓWu"ÏWó?·}xÖ/•‰?æTE=˜T?·}xÖ/•‰3FGL J1921.2+0136@B㭟àÛxÀ‰¦ ¿çÀ8Ý^ʐ²À:û( °z?à÷èόš@…#Ôñ^}@º 3§!¿çg.ÀæBG¿Ø¿›¾Ycì¿ä`U£ª?¿í!5ÜI±>PSRpsrPSR J1921+01?²Öb…gT?¶¥Í=?í¥3½OS?¶¥Í=?¾?£žÉ Õ?Æ[nZ•y
?ì8Œ&Ëæ?Æ[nZ•y
?Ùæ1d D»?Àƒ8ÁœBe?ãçM¯Ý¢?Àƒ8ÁœBe?׉jñšÌ—?¾@吢Q‹?ä;J‡2™µ?¾@吢Q‹3FGL J1921.2-1232@8ô¢€Èè<À(u¡ueÀ98äŒÜòµÀ;A_~Ù?ᓧº[(@b~Ù$@Ihßg"?ìíbM@êE¿á-V>>ï¿â2Çc½{¿ßڈíÇCAGNbllTXS 1918-126?ï
ÁÈ:€?9#u˜D?ž§Æÿ˜¯ó?9#u˜D?è1b-"?Ð̌Ld¼U?Ï:wIùïé?Ð̌Ld¼U?í5";šÁ?¤jnàŸ?¶S^')û?¤jnàŸ?ä°|Í<ß?¼õGÔÁb?֟e‡âA?¼õGÔÁb3FGL J1921.9-1607@5´ß¿ØÀ+Èô^â
§À8ý»V'ÄÀ:òéû±¼¦?仍_Ø
v@V;mê>M?ùØÏY§f?欄ñì†?ËA~ÂRË¿Ø	žBI¿ÏjØïx{ðAGNbllPMN J1921-1607?ï܅Y#áö?ubcZjèw?q½Snv?ubcZjèu?﬙ Åbò?'D)÷K¿)?"ٗΧC]?'D)÷K¿(?î鷺ç­?"éëp?¡´Q…3?"éëp?ïßDèý?'Æ큦!G?œD}à[?'Æ큦!G3FGL J1923.2+1408e@HŽá@!X?¿ÝŽ™¿óå.À5É'm,SÀ9'Óˆ¨°Ž?ÿdF0eùY@ñÔÌËu4?þ«äÐ(Í¿Ø3)˜—¿âÏ^w"›Ü¿âÐ¥Õ>í¿ä®ÀýᗵOTHERSNRW51C?̇[±¼Âª?Å2KIÐk´?èÞ)ÏV?Å2KIÐk´?R{pÃ?qÄ3ïÒ?ïöÂpǞq?qÄ3ïÑ?Ý#=ÓÜ?¸\ôIéî?ánazs?¸\ôIéî?'ëÔ×!Ñ\?ŒÂî@W%?ïh¡YFñu?ŒÂî@W%3FGL J1923.5-2104@1.¸À¦MÝÀ0A'ÿùJÀ7û:Þ"_¦À;1!àûX?ýÎrn²eB@EÍNY?þ6¾¾P¤¿Ø'#_3¿áñ"þÏÿ1¿äay¯XŒ¿ìÒÖ{™ ÈAGNfsrqTXS 1920-211?è2¢
ÈÍ?¾OÂ7Ž)ª?Ï5wÈß´Ï?¾OÂ7Ž)ª?ïÑ{˶2à?ƒÐÒþÚ,"?wB$æ?ƒÐÒþÚ,!?æ&b®"?²9NëJZß?Ó³Ñ:¢ÙÊ?²9NëJZß?ïû©8F%Â?E†AnÁšq?A[çhöÞ?E†AnÁšv3FGL J1924.8-2914@"´ö€$}ŽÀ3œ`ÔV.À8+¨¶mÀ;@)8Þmß?Ó÷#óC@0ƒ¼7©:@F¿×ñÄ¿äVÇâØ'¿æ^òŖû¿ç¶1<¸íó¿å-«eã£mAGNfsrqPKS B1921-293?ïýBOÔûP?=6ŒrÝÂ?5íX%Ô?=6Œrݧ?ïТôÕ"U?‡Sœ)9?w®…•nÕ×?‡Sœ);?ï_Srž"?±<¸sM?"'¬<O|?±<¸sM?ïøcÖþ[l?HõÃÕ¢0?Np¤'O_?HõÃÕ¢.3FGL J1924.9+2817@N篟•\@kDß­úûÀ:p3SêÀ;~ۋ¬q
¿ãP¸t{'@DÖ(–!?þ$º_ÿ¿ïÿûZÔ·Ó?ïÿ'IÏ_'¿Ý©ªFB¸¿Öt¶©R|ØAGNbcuNVSS J192502+281542?ïþbêŠ?&öQáQ?)Þ_Çk\?&öQá,?ï¾6¸Pª¡?"ÏmDìY¬?€rQëÕW·?"ÏmDìY­?ïÈj2õ_o?|ºײ?{Êæ…PHè?|º×£?ïö­l©ç?U2ƒ2á‹Ì?SÒ¥&¬/p?U2ƒ2á‹Ð3FGL J1925.7+1228@Gõ¥À‰d¿üw'áC§JÀ8'rϏÀ:lêÔЦ?à¨I¾B£ò@ëºùe²@Øó_ތé¿×W}ê*o"¿éÊhó‹Ë¿çF:*.î¿é.ð^ÞmðAGNbcuTXS 1923+123	?î‡p<0·O?«ÖêÓ÷©½?§ˆü<ôŠô?«ÖêÓ÷©½?ëdq¤Z?Åëƒc¾ƒd?Ân;óÍnš?Åëƒc¾ƒd?çå¦d¿"Ì?´9V̀Jr?Ð4³6ºh?´9V̀Js?î2Џ:8?œCPž°ãP?§Ò÷\‡?œCPž°ãP3FGL J1926.8+6154@WS*`%څ@3½¬ÿ§ëlÀ8ªlÞPÀ;6w†IZ½?ñB%)[.@Ó;.ª7w?ýÓÁ`]ö¿Õ2¬inÈN¿Û;¿¦@Œ¿Ü4…²uÍ¿Ô¥R?=¾AGNbll1RXS J192649.5+615445?ïþ}Dù?)Ùu±&a?(+¾NÀVd?)Ùu±&x?ï½`ñZã?‰/àÞkRI?€§Ã©|ǀ?‰/àÞkRK?îéBfb"Ï?™¹ÿÌÕ?½?¡kٙÝÓ?™¹ÿÌÕ?º?îqp[ÕÚ?"zTšà-?¨èúO¢¢f?"zTšà-3FGL J1927.7+6118@W0€5D…@3mù³>†À9'&µvoÀ;€‡6À†m¿óؑÇ=@Ó@ÑÌf rý@#oÀbV¿ä=¾bb¿ä
ËHp夿åQ ¤®SC¿àÏ	ñy0AGNbllS4 1926+61?ïùòÀùq?I¯¸íË?H4ÿ=U?I¯¸íÌ?ï۞V½¸Á?{²bñIÖ?r0Ô¡#Ÿd?{²bñIÓ?ï_ŸšÚà+?/¹j¿ªÛ?"¤£úˆ?/¹j¿ªÙ?ïü®³Ã?>&,?:"gYäË?>&,U3FGL J1931.1+0937@GÍÀÓgÀ0î#;nÀ7þÍ;,&À:­?}ÄQ?É@-e²"@縨ã?ýà Éc·¿æœò1¾Ç"¿Ø?R}r¾Ü¿Ür£»Üdš¿ÖN—+™ûƒAGNbllRX J1931.1+0937?ïù›Œr'ö?OZ/RzÖ?I'Î5´/¹?OZ/Rzè?ïe9ÖT²o?¦ÚO?Š?"XÅ5i²;?¦ÚO?Š?ïqÜu=…¨?äf;ó;<?'ÄqXOK
?äf;ó;:?ïù¬Ï'ì?D®ÙÅ6?ILÁ·˜KŠ?D®ÙÅ-3FGL J1932.2+1916@KR ö½?¹†¿ÉÅaÀ7r?«ºbÀ:Rîu"Ó@‹1:Š•p@õi3JZA?ý"ò0±T¿Û ×æÜBŒ¿åÇÜÞÉ`¿êgž~¿íA‰Ï:ÿõPSRPSRLAT PSR J1932+1916?O™;¯ð•½?PÁë‹	CF?ïø±Ú?PÁë‹	CF?(~úWO"V?CËօ ¬¬?ïþxZ‹?CËօ ¬¬?ªâ •Ô‹Œ?¢çË®Sœƒ?îQÕö¢·G?¢çË®Sœ…?@Rʜà;è?4n÷ƒ®Ú?ïûëMXÇñ?4n÷ƒ®Û3FGL J1932.6-4537@v
…@FA-À9ï)ªIëÀ9—*}'ÞÀ;©ôö·â¿ÜøbøGÏÍ@Wª³|D@ "À@øC¿Ú€²[Ìi¿ëbœ#P€æ¿ÔÑð֟çð¿ïÿí ²Û"AGNfsrqPKS 1929-457?ïÿn\É¢p? ԙûì"6?4f˱ào? ԙûì"7?ïØdE$?\?|«‰Íºƒg?sÍÝmàR4?|«‰Íºƒi?îÿš1^Sæ?–3P™Çh¯? \êÁ¨?–3P™Çh¬?ïõš‹^͊?R#(^4j?TÊéBdëö?R#(^4f3FGL J1933.4+0727@F4^ FÇeÀKËè À9Ìò''sãÀ;K®æ1ø¡À47ŸÔq1@"ôW€D‰?ûäÛߏG0¿ïÿöµÿF?ïÿ°²Ô˜¿Ì/'ŠÒÓ¿åSd¹AGNbcu1RXS J193320.3+072616?ïó€$ #¹?[ª¶lNÜv?Xÿ·¿¸Žõ?[ª¶lNÜv?ïEø¢6?ªù"³7?—Gœhë¹R?ªù"³7?ïŠÛH‰Û?†}³—µ'w?I-Ý»ñ?†}³—µ'y?ïÿ}þ¹Ê6?)5YãôPì?@(ƹ9€?)5YãôPð3FGL J1935.5+8355@]ÁÁÖυ@9τ´Ñ.À:9‡aˆ±À<£mWò/¿öxƒ.ž#@"£]'­A@Çó?Ó)³¿èž	㉿à+xÿ›+¿çCú°¿âÚ)nä9PAGNbcu6C B194425+834912?ï_¬´Ÿã"?¡ýëÃÿv+?"
ilh?¡ýëÃÿv+?ïž!;Ý?‡åìDŸÜ?~°ïbq¨?‡åìDŸÜ?í¹ ¹.Wa?¨Úf	ç"#?²6ú6Dô?¨Úf	ç"&?ïöªA­?V¢Œkjl?R«}õؤù?V¢Œkji3FGL J1936.9-4719@uò®ŸðË°À;î€{»bÀ9he˜ºÀ;>`ñ—‡?Îí,öz'@Š+"+ÁO?úAÆa"Ú ¿êü¼Ëfµ?ƒPØ5¿2¿ÕÏ
ž¿ºhÿ{~Y*AGNbllPMN J1936-4719?ïý†)ÃË?1¿(y?3ηÑá«?1¿(y?ïç}ÿO
?s	÷lžÅ?h'ð°òî?s	÷lžÃ?ïŸè¢"3½?‡"óÞ+
™?ˆ×Zó¤?‡"óÞ+
•?ïòÞî_bã?PÉȍɘÙ?ZB#A:;?PÉȍɘÉ3FGL J1937.0-3956@vrìà2ÛÀ9SÂÀð À8ÖϦ›àœÀ;y°Øzù?à4èß
R@þÚæëÝ@fë¿VA«¿æ-Råf\ç¿éÆ@ÓH«¯¿çA#5åA¿éó¨—´AGNfsrqPKS 1933-400?ïþ\!+)?/ÞN²Àn?*=ïíM{0?/ÞN²À3?ïÑ£[;³×?ƒ^Pi1Q£?w.Rb&?ƒ^Pi1Q¤?ï',RÓ?†óçåžÁ?‹¾ôüëK?†óç垽?ïh<ÄD77?'É6ûÏ?'øgwy;?'É6ûÏ3FGL J1939.6-4925@uÏ¿˜0äÀ;ÜLŸëÃ2À:5¢,RƒÀ;ŽŸ–2ÜÌ?éù·ê¬%@
Ý,µ?½Z?ùüÿ"µb¿î&µ´NÉ?ïþÖ¥œ9æ?žØh-Þ,¿äèòÂÕ¨AGNbcuSUMSS J193946-492539?ï͊«Q(Ñ?ˆí¿4ÎV ?y:ªWk—¯?ˆí¿4ÎVŸ?í|‰í¯Ât?À©9Ðú
?´°'ì]?À©9Ðú
?î¬I­ÌÑ?›39¢È(?¥>e#2â?›39¢È(?ì}Åö<ö?µB9÷¨h^?¼ÐK–P?µB9÷¨h_3FGL J1941.2-6210@tèWÿ›V2À=…êÀӚFÀ8´wM>w4À;xv̗?íõíqL@§[-M@%@u¿]MŽ¿Û[-3{׿æU™ªû0¿åIUÐRN"¿ì)Ø`Ô¬AGNbcuPKS 1936-623?ïí‹j`2ü?aŽé(	M…?bt•ŸÍd?aŽé(	M‡?ïÞrr¡<?x•æڕq?pÆðƯa‹?x•æڕs?íg&ÁÖ¥Ú?£Ü™[㠎?´ÆÉñJÑ-?£Ü™[㠎?ïÈÓÖÌ?mÉ¥êÔÍÀ?{–xÀ™?mÉ¥êÔÍÀ3FGL J1941.8+7218@ZÁ?ÐÐh@6ÀA¤À9]þÀdßÀ;Ÿö\OŽ?ó'-ªP@L÷¥¾k
@Z9¿¿H*¿ã•ó‹¿è"}š¬ál¿êISäŒ:¿ì–a\Ö¥AGNbcu87GB 194202.1+721428?ïÁ~®;iÎ?"‹yq°?@¨âK3?"‹yq°?ía2…ý?º•
(¼þá?´÷WnkÐ?º•
(¼þà?íW&|Y£È?¥d¯÷€"?µFÌ2áÀ?¥d¯÷€"?áþõzM:?½$B97õ?ÜîeŽ?½$B97ö3FGL J1942.7+1033@HÝ Y§;ÀuÈ@K·À8:Cû"~À:Á'h$¬ˆ?ïÃ|"jÞ@Š)åË?ý¦?Dc‡?¨lÑir¿ÒÛz,Êký¿ÝÍؚ$GÍ¿Ûܟ†K;ÆAGNbcu1RXS J194246.3+103339?ìÅG«¦+ñ?µ›ô'áã¹?¹Õ¢Π{?µ›ô'áã¹?é^–ï›'í?ÎßD9§P?ʅ¤A'´I?ÎßD9§P?ëK÷0¹
é?¬{Îÿq?ÂÐ#=Ô`?¬{Îÿs?æ
pÝ"é?µ³¿«Š?ÓåE»ú-?µ³¿«Š3FGL J1943.2-3510@ƒ/ÀÀ93_ý–™À9"ÞFqÔYÀ;‡^¼Mùˆ¿ÁˆÛrú?ï@b•ZDÅ@Â@+"-¿âÀ'Æ…z¿éèF>ÂwM¿â¸%ÔX¿ïÿʓ6©	AGNbll1RXS J194306.8-351001?ï÷~xƒ0ù?c
1ZüÕ?Qùžé?c
1ZüÏ?íÀ×gßÂ(?¸îÆ=·r"?±ùDÁî²?¸îÆ=·r"?îKm°Ë›?É"¥]ÿó?«I$óFO>?É"¥]ÿñ?íÕxîX'? þy²â?±T? >É? þy²â3FGL J1944.1-4523@vAà?pXÀ;ڙ÷LÀ:²ÕíݾÀ;Åëõ‡:?Õ¾°>÷Œ"@
MYÁ<uÒ?øô­ÿ'+¿¿ïSZðç^?Är0ìSr:?¸
K?eè߿ڔcl®KAGNbcu1RXS J194422.6-452326?ïû°Œ>qI?>í­†âLŒ?A=Ï:Û?>í­†âLx?ïÝíï™?xÒz.—\Ò?q|‰p³?xÒz.—\Ô?ïw£öñˆ?†»
_¥ËA?Œ"Cž?†»
_¥ËF?ïÓm
*´1?w‹–$O|?vIzê¥æý?w‹–$Oz3FGL J1945.9-3115@!Ø,àèÀ8"ªKÀ9-Ë)^žÀ;kÇc€À]
ÐXó@àqŸªÆ@̂Ÿ­¿æ¦;r®¿è¹áaÅ¿ØÕ5¿åÍæŽÙ¢AGNbllPKS 1942-313?ïòÊ/ÇI?]ðˍּ)?Zk¡þqo?]ðˍּ2?ïæô¹ƒšÃ?s.À^_?iF|e>d?s.À^^?îÝ¢+åßö?—.¼l×`?¢%ÝA¢?—.¼l×c?ïÿÄ7Û0¼?NÒ<V{>ýäg¡Úy?NÒ<V{u3FGL J1949.0+1312@I«?ÚácÀŒ,ºËCÀ9²A'è|VÀ;A'¡ Ï?àäß@ƒå"¯‹@KxßdÔì?ïÿƒ¯]·Q¿ä7¯JA'ú¿æÌ°i·¿Öý¾Û%3AGNbcu87GB 194635.4+130713?ïôF¯‹ž?aÃ]:ÚMÝ?Wr éòÅM?aÃ]:ÚM×?ïŽ'Û?¨é~jM¾?ŸÎ=ǭě?¨é~jM¾?íàn.#˟?£²r­oÉB?°üŽŽá¢þ?£²r­oÉ@?ïteÊ1i~?†`"÷'ý?'sF¹ÒÐM?†`"÷'ý3FGL J1949.4-6140@tò$ p¸ÐÀ>yn Ç‹DÀ:Vû…Fü>À;º%—i=±¿íÕµ‹"h@Œª^¸È@vý §•[¿í5}€¼Ür¿áÄ´ø@'¿×4#H.˜¿êç…-YˆAGNbcuPMN J1949-6137?ïîóë"-þ?cÍø94ÿB?aÝÒ÷?cÍø94ÿ=?ïêÙ¨îÓ¹?ojLŠÒÀ"?e&W,G€?ojLŠÒÀƒ?îU¼BÁÀ8? Wä?ª¤;Óãün? Wä?ïý/4"ñÝ?5èÚc'õ¾?6†[`q}?5èÚc'õ×3FGL J1951.6+2926@Pjå?õ¹U?õh?."À9R"狔ôÀ:é'üft?ö*åS×B@T+ê¿|?ôg ÈÍcÌ¿ßs©$Ññz¿Þ'0",J¿èrNÁÙÿ¿ï9ºHfOTHERspp?KðO,µ4?N[ó@"ç?ïùìôÓ?N[ó@"ç?u´ìZ]?¤Ó¢¼té?ïº)/€N˜?¤Ó¢¼tê?¥'BSBÅþ?—©™	8?î§ÛÚËÓ ?—©™	6?±@£ïÓ?£ˆS¥F?íß7ý‹'?£ˆS¥F3FGL J1952.9+3253@Q2	ÀÂl@šñ`*CÀ6œÔÞF.À:›™[†8"@¯A"4Ø@'©«µz÷@Ná¾\¿Õ²Àe¡'¿á(ò"OhÒ¿æ{"噑¿ìèj"U¾PSRPSRPSR J1952+3252?4r	ñve?1á×åyÓd?ïýlQ¾ÁÑ?1á×åyÓc?4Vñ?F®'Ð\P?ïýu<}Ý?F®'Ð\P?záÙ,}O?q ]?³NÒ?ïÊ<Mû§?q ]?³NÎ?{¶‹ôµ	?ú.92à2?ïÿ4"K Z?ú.92à23FGL J1954.2+2836@PO­K6?؀ǿáp¸À6ó®«y•îÀ:QÏng¼¨@æa³Ï$ì@ÎC°.@»ò¯Šq³¿×$Á®"0,¿àËÁcj¼¿å xðÏþ¿ì…i/ˆG¦PSRPSRLAT PSR J1954+2836?4•8U/¨?1{q"¤e?ïýmXõZ?1{q"¤e?$[˜Fœñ?>¦ÖÇLX?ïþºF{–2?>¦ÖÇLX?tF3ª?W2ÜÍ÷F?ï×sáÑéš?W2ÜÍ÷4?82VR¬òL?3=NÏÍ«Y?ïüùµ5ªa?3=NÏÍ«Y3FGL J1954.8-1122@=¯@Î&iÀ3(¿ó vÀ8d£zÃë}À;Oß;dZ?ó"ýèù~1@eSvŸ™Ž@+"ÿѱä¿ã=/!î¿âÝ@Š´¤b¿æ»j¥Bø¬¿çä¢WNAGNfsrqTXS 1951-115?ïµÀ|þ?€‹@ÁO	±?'ù ß€Å?€‹@ÁO	²?ï¶0'¾×T?Œ$tû7ǖ?'sßPJ+H?Œ$tû7Ǖ?í/±¡ýƼ?¥!rÚaË·?¶'rðÊ)?¥!rÚaË·?ïG‡| os?†ïRñ0¿ñ?—{òh?†ïRñ0¿î3FGL J1954.9-5640@uOº¿¹¾ÓÀ>üfß2*À9ø&yçL«À;¬&è¢i?ëáß͟Iv@Iè"Ïf?þ
•µ¢º¿ê³À;ÄÒ-¿æÙ~*ʦN¿Æ²˜£-Ž¿Ð¾cÓd©AGNbcu1RXS J195503.1-564031?ïü0Edb ?: DÜÈù³?>}ÔÜï«?: DÜÈù§?ïÛ}Ñös?|?‡©M|?rAûÅó?|?‡©M}?ï!5?ï‹?')w[ˑ(?›ÙXB¿?')w[ˑ,?îÛßóc?•‡aáiÌÓ?¢BÉÎ?•‡aáiÌÓ3FGL J1955.0-1605@9 1ôoÀ5"
`:Ó;À9qá/Z`ŸÀ;^ꉯA¿à\L'ª@†Õûõ"Q@`=;"¿ßÍã}"S¯¿è2:àÚ(‰¿Ïñ¢Ål¿áû¶¡+"1AGNbcu1RXS J195500.6-160328?ïç㞏`?q0줶ߟ?haæpŸ–?q0줶ߠ?ï½ÂŸy.ž?"Qøwà?€X!´X~?"Qøwà?îŸïO¾Ùã?œ	a¨Ù
#?¦aÀ?œ	a¨Ù
!?èV¢?z¨Nﶌ?~¿¦‹Ô¯G?z¨Nﶉ3FGL J1955.1+1357@J^à€øÀ;– oÀ8áú"pmPÀ;6¬¯öÓ1?ï³–&@,ëp{é@é@kU¿ßÿ¦"÷@¿æE9BkàN¿á
ЬÅ	N¿éÓÇùåpAGNfsrq87GB 195252.4+135009?ïóƼk¯—?Wُ	#Ã?Xr‡( Ôû?Wُ	#¿?ï<àö"?®mÁ¬só2?Ÿ½8cá-Æ?®mÁ¬só2?î9˜Ô¾Lu?¡9DMº?¬fr´8¤?¡9DMº?ïÉpún–?lžJ†fu?{Gò'È´à?lžJ†fu3FGL J1955.9+0212@E8"åx•À*ƒõž}.)À9÷Wfï"bÀ;o³1fª¿ó*ü6i@
œs]ð¡?þÖ
€·ux?ïøjb§ó'¿ãC_T	¨±¿â.­*M¹û¿Ó`óí»
AGNbcuNVSS J195547+021514?ïú'¦$¡t?Hb±t¿Z²?Eµgmz0_?Hb±t¿Z¶?ïÎx{1?†Z…"I}æ?xøÃÂqg´?†Z…"I}ç?ïPRʤ÷…?Œa	™ÀóÊ?•õ¦«ac?Œa	™ÀóË?ïýÝkÙ?7cø 5Tî?3ñ¡7—?7cø 5Tå3FGL J1957.0-3234@ "´ ©ÓÀ;4À_×,À9Åþ¦c¬xÀ;€­-¿ãAði\@s³û¼?@§Å_ÆB¿às¬ûԪſïþՇuC"?ï¯d3[L¿ä_Ë~GŒAGNfsrqPKS 1953-325?ïû°rÂ×?Gi¶¢wöŸ?A?Š4ô¦y?Gi¶¢wö¡?ïèÚuxXp?qoËaáÊ?g%Š‡§©?qoËaáÉ?î˜Û:|=P??~…êÖ:?¦rLX<+
??~…êÖ6?ïýeIkI?TG5[§?4Õ´¥·êX?TG5[œ3FGL J1957.7+5034@U&¸`.>@&G^cb¦À8(ÂÂ#&À;täǕUg@ÿ¾Šêª-@ò/@µQÜ@—çZl³¿ÝŒr'¿–¿äÒBR5¿í;u-meM¿ïÿK<igÎPSRPSRLAT PSR J1957+5033?°¨ÇÐÛ0?¹Îƒ/­²}?íêüçä›?¹Îƒ/­²}?`q'Iøú?iuCSÇ2š?ïïŽ}¶ø?iuCSÇ2š?ÂCjº6ã?°åpÕfÖ?ëo%z'rH?°åpÕfÖ?3œ‹†Bˆ-?6ãsè"pý?ïýŒn7¯?6ãsè"pý3FGL J1958.0-3847?ø¿ÜÿŸÝÖÀ<úéŸkj²À8ƒêìÀ;GX&1Âñ?ö/R֑œ @ß*òœë@I1c$g"¿âͺPy¸¿å'¾7³ ¿çe"·'Üo¿ëxû¿S'yAGNfsrqPKS 1954-388?ïĸ?{)Fff?}ÿz#ðqÂ?{)Fff?ïå³G
¸Ç?sš%ª%?jL¸õG8î?sš%ª%?í
ɚù²?¥¾Ï{9°Ý?·©³(2o¿?¥¾Ï{9°Ý?ïæº>bh?cÍWçà9?iEÁ睘_?cÍWçà=3FGL J1958.2-3011@%åéÞU‹MÀ:Ǎà'ódÀ9×Ç.'Z¸À;h†`Ô¿©ñ/H;.ß@œ€9¡6q?ý²³?ê•œSÞ$¿æäWôÄɯ¿Â·è"cQ‰¿Ö|âž43AGNbll1RXS J195815.6-301119?ïÿ«>h¬?ÐeayÀ?0{%Ôû<?Ðeaz¦?ïåá¶5U?s'µBîÌ?jIäʪb?s'µBîÏ?ïØíéú["?z1iÇûd?s‰Ò6#?z1iÇûd'?ïühÌ1*"?6zaj?<¹žv«Z ?6za~3FGL J1958.6+2845@PxèӔ¿Öƒ×`#¬-À7	.Cà)¡À:o9ä'\@æZSÒ@'€ÊjÇÊ?ÿWS–€	¦?<gºNoû¿à`ïë¿ç¨óºÞsú¿ë¬êŸ·çPSRPSRLAT PSR J1958+2846?`lÿ`±ù©?`)
–ȸ?ïï"ŸN?`)
–ȸ? ùñ:{`?:©td`‹?ïþð`ìXI?:©td`‹?›suXÊk?œ-ß×õj?ï$dU?i­?œ-ß×õj?(Œo–/ü?"£}V_Ê?ïþw9?"£}V_Ê3FGL J1959.1-4245@vQð€0<À=üÀu¦uÀ8šw§×IþÀ;~×¢äß?ð5b]]?@Æ&ö¶@Å»à~í¿áíÐGMû¿çB5×Ó;&¿æ`,,¦®¿ïn1–¥ôFAGNfsrqPMN J1959-4246?ïð]¯§öQ?Yc•!|™ö?_D °[°?Yc•!|™ÿ?ïê~ôp…š?p¦×Âg?ezf·?p¦×Âg?îýTÀ«N?•žÞ(@? *·õK?•žÞ(=?ïïö¿v¹I?Z<˅¡Ér?`	@‰F·F?Z<˅¡Éx3FGL J1959.5+2047@M—ç@™ÅÀÅ)ÀBеÀ8¾í:*ž9À;2šY²ù½@)ï¶Ü @>2«#æ?ÿbxò)(¿Ò¼·µ}>´¿áæO̊Ìf¿é͉Ñ`Á¿ïÿÕOþ"PSRPSRPSR J1959+2048?móðÂs?xÇã?¿ý?ïâè=ù?xÇã?¿ý?LªôYÐ76?[Ñú³ãYø?ïøÕBé‹ó?[Ñú³ãY÷?¤ª|ý;6?žHÒ?î¾5X0,M?žHÏ?]¶jK(?§?Ly[9=?ïñ$ÊÚkâ?Ly[9=3FGL J1959.8-4725@uüÒ}ÔAÀ>Û'ÿùJÀ99ôêù¾À;D$¶˜­á?õÚÛö¶U<@9Üùë"â?è1k©,šÏ¿‡Ç·—¹ù¿½	[]ô§Ý¿Óâž/Ö\n¿àSݦ6AGNbcuSUMSS J195945-472519?ëޒ¡÷ü?¿ªvâ3?À…·íx ?¿ªvâ4?è/cØDÂe?Ï£¥7º?ÏBpžìöm?Ï£¥7º?çªÃWF´?·"j)'?ЪyQr—û?·"j)'?âjw5o'?¿Õ!á&«?Û+• Üá?¿Õ!á&«3FGL J2000.0+6509@X€Ì¿Ì3J@1ª_ÏspÀ7h¢q¯oÅÀ:¸aÏþ°u?¤âÛÊƬ@B"FY?þ!±á9u¿Ù¿Ìhù¾¿à2'U†ß¿Ú´Oñb‹ï¿Öƒ×¢¶PAGNbll1ES 1959+650?ïûûQÂ?HTª©-0?C¨¹¼üÑ?HTª©-0ƒ?ïݽHu¾à?xjjgCÎ?q![Å £?xjjgCË?ï³ù¼®˜P?…Ž½]ŽØø?ƒÔYìD?…Ž½]ŽØú?ïù<ĕ;|?Hʸ@¼¢ô?Kí«é?Hʸ@¼¢ÿ3FGL J2000.1+4212@SaqýÌI@ªE`zîÀ9A›\è8cÀ;!ÛjõA`¿òöƒ—¤¡à@ÅWìÐù,@¾3Ÿi½3¿ÞšXFú ©¿ã¨ž÷k÷¿êŠ"ë"çû¿Üö§‰‹AGNbcuMG4 J195957+4213?ïãnaHÌ?pœ
Vã¬Ø?l'ž·ç3v?pœ
Vã¬Ø?ïÊrº!y£?Ž@'fÕ¾P?zÆ¢ïC.`?Ž@'fÕ¾R?íùɗ\ØV?¢Þ7ú±?°1³E=J?¢Þ7ú²?ïüäxÆð·?9VMrõ¨}?8Ü9ÈzJ&?9VMrõ¨œ3FGL J2000.4-2926@'Íä ¦hµÀ:ÿyŸÿhÀ9WMî \+À;jE­‰:§¿Õêú†÷ß@c²åE°@ÕúÁ;t¿é†pÞÓÇ¿æÞSèO¾¿ç«v-ƒÆÉ¿Ë1Æñ~YAGNfsrqPMN J2000-2931?ïæ^ÜÊ»?nme®ÀZÒ?i¡#5Dòê?nme®ÀZÖ?ïß+©þÅ?€"œ€YÍ?pj+8Å?€"œ€YÍ?îYøOãLe?ž¦jƉ¢3?ª`{Ë9˜?ž¦jƉ¢6?ïلFç4?l=c
±þ?s=÷\Œf,?l=c
±ÿ3FGL J2001.0-1750@7ýJ€àÀ7%A` JÀ8…Þs¾=¾À;G¯e³¹¿ÙLAþcXü@¤Ð.@z+µ—Ò¿â@0œªñ¿èö‡Éëúm¿Úê"65ú–¿å"ì0•IAGNfsrqPKS 1958-179?ïÿáºüü}>ì´ÿ飬ÿ>îEV`>ì´ÿ飭¡?ïè͵=0?wÕ't l?gá2JÂÍÇ?wÕ't l?ï×Ö1&]?vy8žÞþ†?tç}lш?vy8žÞþƒ?ïÿš§JÉ×?	jrÒç–?	V-M‰Ð©?	jrÒèï3FGL J2001.1+4352@SÄŸê³@s•À8–À7Ô¿ª¥À:k$;H«?ÓH îÀ›@T/(6ªâ?ÿŠsž³3ô¿àù ÀTnl¿à8îCȊ¿Û:K•Õ"Ç¿ßÕü#°AGNbllMG4 J200112+4352?ïùA9r^
?OÍìW¥T?Jû6‡Ó'?OÍìW¥^?ïÍͺí[«?‡éè~Ù?y"‰R+6?‡éè~Û?ïq[—¿ƒ1?[áܼ?'ԍ™Ý?[áܽ?ïþ´êM‹?'¥öý,û?$·['E\?'¥öý-A3FGL J2001.8+7041@YÕÑ_ÄÖ@3õÕߛªÀ9‰´	‡h?À;""²Çì?à̈́ò\@
‹oK<ih@§`¥aÏ?ïŲFŽ¯±¿ä—¿iÉ¿Õˆ&xqi¿â:&ù$TÚAGNbllTXS 2001+705?ï噡y•?pèÃÚɞ?jf^û†j¦?pèÃÚɞ?î"S5=?«Áà>¬s?§ºÏ,¬1?«Áà>¬r?Hxvð?˜_cÜ:cü?¤ÖKxxì?˜_cÜ:cú?êúH88•?³•¹µ?Äßù«?³•¹µ3FGL J2002.7+6303@X
FŸ÷¬@0oò ClfÀ:i¨+,ÔtÀ;á|lb(ê?㙵·÷'@ý&±ÅŠ@#¿¢Â¸¿ä¡?[pz¿ìÒu³?ÀÔjÁÑv¿ÚsÜ
­XAGNbcu1RXS J200245.4+630226?ïü¨6$ ?=š¦?LÒÿ?:¾NßÞúP?=š¦?LÒÕ?ïÑjørÝ*?€Ó£»	ì?wJƒÆ'ku?€Ó£»	ì?ï"íÓrRM?ƒ©;Ê>ª‰?‹‹#klÓ?ƒ©;Ê>ª‡?ïè•©?i?Š'Yƒ\?ˆ…Ú•°%¿?Š'Yƒ\3FGL J2004.8+7003@Y¶Â!y@3téÅ+À9ò	7´À;‹ ¬Gò?°Ð®q¬x@ÏÇÓé¢?þ©€Â]2¿å÷\UÉé¡¿â§ÆZÂÄ5¿Ü¼»ŽrÊ¿ÇâzwÚAGNbll1RXS J200504.0+700445?ïþl՞à?/"ÒK¥g?.¹2¦à?/"ÒK¥9?ï׬VÁ
~?~'hì!?t)ԟyA…?~'hì!?ï֛n:Èå?zã'LÝ?t²H⛎?zã'LÐ?ïñƒ*á?S¾7ïMŒÒ?]ÓÒùª=Ë?S¾7ïMŒÔ3FGL J2005.2+7752@['¡ Ï@6¿¤Ÿ‡dÀ8š°hÀ;~¹Ù«?ôÍJtm@Ët‡ff;@¿Ý¿ŽJÜ¿àã?˘¿ãÄÊPà\¿á©ðìçŸa¿ç¥eµ2ÒAGNbllS5 2007+77?ïø¦XãlÆ?Q'=¥Ä?MfœrLâf?Q'=¥Ä?ï×/4?€zø›?tsheüþ'?€zø›?îHƟzÂ+? ýÊòC?«s–SÝI? ýÊòD?ïÎÅTG,?päÒÛpZT?xùUÜi»?päÒÛpZR3FGL J2006.0-2311@2ø÷àvͽÀ:-Z@¾61À9/?ÐÐgŒÀ;}|Ùor?îŽ"é+@hö'äöd@ö?ŒÝÉ¿áØp+â¿çrDoè脿ë™IÙõL¿æúÓÓ§1ˆAGNfsrqTXS 2002-233?ïþ7Êòa?)SH2™–?,ŽãPÙÞþ?)SH2™B?ïÙ·Pë»?€m2Q®e?st$WŠ"…?€m2Q®e?ï5œL=·°?iоËÆÁ?™LvxI	ý?iоËƾ?«ô"?'³0:íÉ?ŒR•Úø?'³0:íÉ3FGL J2007.3+6605@XÏè?ïÚ@1n´_î}!À9€ú:þÀ;'-±2ã?ÚQð"
yÌ@VÆwÉS@·ò ¿ãn×Ѹ™å¿ê°Ïb «¿å0Ì6àøå¿ïþ•2ñ]ÀAGNfsrqTXS 2007+659?ïü0YŠ½?=åʎ܃È?>{3ª	?=åʎ܃º?ï*Æ弉í?ì]û\çò?š§#Hn€?ì]û\çò?ï"gaaÀ?‡êÃéTµÝ?‹&'½çB?‡êÃéTµÖ?íÀI+p.?›íLù_ÜÅ?±ý¶¤~ð?›íLù_ÜÅ3FGL J2007.7-7728@sË/ŸËÀ>Œ6`]'À9sÔöfú
À;›wï$æi¿°áõ"x'@ÿÀ+©§@výòÿf¿èz'V?ñ¿äòu¥Õ¿é¥þÓôÎ
¿ïÿ?9!AGNbcuPKS 2000-776?ïüEWü®?C"0"'??5Õ@•Ú?C"0"'?ïÞ&öõÊþ?x_úÙ
Ï?p섅€ù?x_úÙ
Ë?ï3ûY÷-"?'Á}*Ðރ?™€"Á[Í?'Á}*Ðރ?ïÉl6ñÕÆ?p›&þy›½?{Iä‡P?p›&þy›Ã3FGL J2007.8-4429@v6Ê?‰'ËÀ?ÕŸÕó½À9ŽTEÒr(À;­†Q¾8µ?ÈE'² ¤@F´šQ@¿œÿªšž¿ã>w"k4¿æä,J
æ
¿ë:ï.˜ç¿ÙÁ6ÓÉÆAGNnlsy1PKS 2004-447?ïúåšÔÞ?KqW•XÐ?Di—Œ¬‹b?KqW•X¿?ïãm	 "0?sú,ô]?l'ößlÍó?sú,ô^?ï£4YŠ?"M²ÉA?‡2ÿi|ˆ?"M²ÉD?ïƒå	¬à?"‡êü÷tâ?¾ý"Çè?"‡êü÷tâ3FGL J2009.3-4849@uæ
 '§À@LZ&–mÀ7ӊë€ìúÀ:©³%[Ú¿íükl@@€¦Kٝ@?ü_ãìŸP¿Øfû"¿h¿ÛvÞX»X¿Ö2ä%Pi¿×-	þ±vZAGNBLLPKS 2005-489?ïÿošV•Î?tùTI@?µ-FA ?tùTI¥?ïîÌ:ºÓA?lÊ>å@2?a3ÅE,¿u?lÊ>å@0?ïÎ>A"J?€+ͺsý˜?xàßnñÚ±?€+ͺsý˜?ïÿş0§é?®-P8>ý0g¬I"?®-P'3FGL J2010.3+7228@ZVhÍJ¡@4$WÀ±5˜À9`¬é·À;Øwûº ?ö" =͕õ@Š•DË6@£3ø€ñ¿áí¬¼ó!1¿ä+ÚûIóû¿å{ÿUò6$¿ëêHeì»AGNbll4C +72.28?ê¤4÷
—Ö?ů./ö?Åo,#É ­?ů./ö?à(CöÏ?ÊÜ¿©Í)Á?߯îßxc?ÊÜ¿©Í)Á?ã¡ZMëÝ?»×?9²¨?ؽ÷Kd(G?»×?9²¨?Ó1t.Ç«†?¯[I"i›j?ægEèœ*=?¯[I"i›j3FGL J2012.0+4629@T"GŸÑÁÿ@ƒ32ÚÀ8PݝÕh}À;<äŒÜóÀ¿Ï+šã@Œ=AT@@Ü= ŸrL¿ä©‰[¿ã÷Z4,¿Ö?H=9$¿ã0I'f2uAGNbll7C 2010+4619?ïÿmão?íž *?Cœòzv?íž )q?ïÚ[ù1K–?ˆ‰¼â:o?rÒgZ4©?ˆ‰¼â:o?ïÍ/"ïß»?€|ÚA<Ò?yh=ˆ""?€|ÚA<Ó?ïÿø¼K"1>àÓÎ+$v…>Íѯ;^»>àÓÎ+$vÕ3FGL J2012.1-1643@:=ÓÀíÀ9)?O¡(À9´a¼æÀ;°}À?`?û+çpÌ@¦5þ¿Ž @æsžg}¿Ò&ÞJ<}ù¿ì—ÁÜȇ2¿ïôƘw§ú¿Ùú39Š²˜AGNbllPMN J2012-1646?ïüÏݺOX?Ižo},?9-…:×?Ižo}+ü?íœHé?ÉèÐðˆ?·WK¸·?ÉèÐðˆ?ë3åüÕA?­?c®ñó?Ã0hªûê?­?c®ñó?àô»Ë?Ì"'ŠnªU?Þà‰éØi?Ì"'ŠnªU3FGL J2014.3-0047@Dýžà*w£À2ºÜ fèÀ9wU4åºÚÀ;Fù	q?Ø&‰åz `@5dЏ$ ?ýP!?Àµ?ç]G¦²±Ä¿áÙÅ(yØ¿Óè}†­G¿â'²Íƒg9AGNbllPMN J2014-0047?ïûa‰¨<—??"Zà·È?ByÙ_
«??"Zෛ?ïÂϐSÈ?‹åõ€z?~˜7Öó?‹åõ€zŒ?ï¨(±¦Ç$?">09áF²?…õӖN6?">09áF®?ïÓ?6TÊ{?gºâ*X÷?v`d՚Áó?gºâ*Xù3FGL J2014.4+3606@Rw	ÎÒa?éƒ9õÐôÀ8íaö•À:i"ïQ0?õ'2T»ï@xq5¢NI@0~ÀzY
¿à	Ç^ÎÂp¿ã­¬`›¡1¿ë>H:+tù¿é&¯â[TeOTHERspp?`ACFáÛ%?rXCýëÁ?ïï¾¼¹%?rXCýëÁ?'þ½ýÌã?±åhڐ½á?ïw
š?±åhڐ½á?À
Ž@hÝ?¯¯B`Û­?ëüœoåý?¯¯B`Û­?``\¯´Ø?'qSLë?ïüý'Y?'qSLë3FGL J2014.5+0648@Hw V·À.€LÁzÀ9o>À;T' ¦Ô¿Ú}ôÌ_‰@fSvt¦p?þ¤®àþˆ?çW­ËÕ¬¿èU‰%û^¨¿ÓïKº
ß¿ÙvŠq™±~AGNbcuNVSS J201431+064849?ïüT<R[Z?>3Z$ïà?=^m%,—?>3Z$ïî?ïÉ}È©^â?"/€‡V®?{A«PŽ½?"/€‡V¯?	Ê?'ö»…z×?‰Zú:ý?'ö»…zÖ?ïòƒït?WwŒ±Âöv?Zùâ!æ?WwŒ±Âö}3FGL J2014.9+1623@L®¡@W%À$;ÿwDÀ9Õ(X䝤À;qhµËÿG?ºâÌÆö&Á@%2?@G]Ÿmn¿å‡'(Ap@¿æQ(óØï	¿äýt½1­¿Õ¬s¦jãNAGNbcu4C +16.67?ïê$\§?rŽ¶?eÛ£üìXÔ?rŽ¶ý?ïR†s‹?¢™ÖIz ?•¯?ñŽœz?¢™ÖIz ?ï[µÂ²5‹?'´}˹?"‰G©¹Nµ?'´}˹Œ?ïÍáƒÏ?mÜð#BT?ywv>M?mÜð#BR3FGL J2015.2-0138@D§:¶~­À3XhÌÀ9%¹˜<¢HÀ;^||R`ö?ì8_Œ¤àí@
Í,݃©B@7* ís?±F(mÝS-¿åð"Ò.­à¿ã‹ü]¼§C¿åRÜN[>AGNbllPKS 2012-017?çìJ-fé?Ê<fwÏ^R?ÑÞ'k¥2.?Ê<fwÏ^R?àµB¾Ÿ?Ó¡ð‡æ´?ޕz'Áýä?Ó¡ð‡æ´?çwàlԀŸ?´™1Éþ™?Ñ?&Vþ¿?´™1Éþ˜?Öjς"ßþ?µÎ{ÛêÃ?äʘ>î?µÎ{ÛêÃ3FGL J2015.6+3709@R·_ßÏ?òø
€CRÀ7Ïng¼¨À:+l¤nò?ÿµðÓ×@rõJð>@@îݘͿáÞ³&¿åÂóýé$q¿çxýP/¿è¤ï‰ÌXDAGNFSRQMG2 J201534+3710?é×GeBr?Á·üìªÊ?È¢âjö7¸?Á·üìªÊ?éœÂüõb?ÒBÇÆ$kF?Ɍô*uÌ?ÒBÇÆ$kF?祮FþY?´ï.¢/T<?д£rMì?´ï.¢/T<?ïòev9?¢o	ùí?Ÿa³Q8Ým?¢o	ùì3FGL J2016.4-0905@A+©Ÿ¡—À6úã Ì(bÀ8ࢻž§À;Bqÿ÷œ"¿Û}ˆ¯šœ@šÍ¥å­C?ÿÀìÿÈ!¿Ý(§¶_D¿ßÙ.ÁÌk¿àFbuž›?¿Ûj?ZD*cAGNbllPMN J2016-0903?ïþÈŗd"?$"j¹
b?#s¦‰·š?$"j¹
n?ï㕸ó·?xó_nf?ljGHÿX?xó_nf?︱ x[ï?£·j{Œ?Ó·áé?£·j{Œ?ï÷¼Âãö?L©qñF‡ƒ?QĆz8°?L©qñF‡˜3FGL J2017.3+0602@HOt cLÖÀ0:?–îÄÀ8"úgðÀ;×@Än@ƒ–ÿ‹eú@
S
ã2ê¹?ö'ª%Øם¿Æ‰Wu:rJ¿Ê£ö¿º¿Ü÷ßFïJ¿ìÁÄÜq
<PSRPSRPSR J2017+0603?I}âR+~?Em]Å?ïù ‡k|6?Em]Å?aK.ÛÂn?j,»ê²ÂT?ïî´Ñ$=û?j,»ê²ÂT? ‡ÐFg3?Ÿhh(<ž¢?î÷'û™ŒÎ?Ÿhh(<ž¥?F	7Ðظ??›‡Š:š?ïú}²Éü??›‡Š:š3FGL J2017.6-4110@vz4¿ÍhÀ@À?öÀ:få2õÒÀ;ÉdÞב¿å	 Å>ÛT@
Lº–@FônJ6¿ÛýxU¿ìæRµöп´U¶ÀÆÚ¿Ïš¼ÀvAGNbcu1RXS J201731.2-411452?ïÿ·Ãá–? ‡¯©³?<Gš– ? ‡¯©#?ïìüí­®?lµKÕ&m?cðRRÉ?lµKÕ&k?ï0¬¢?ƒÏ¤¾?ˆ³ûÔû—?ƒÏ¤¾?ïþh¥!™$?'*cf¨Û?)u­æmÈX?'*cf¨ò3FGL J2017.6-1616@;F'À9@"À:7{ßto>À9J
'/ï²À;rÁ3;–¯?ðºÌ1qg @Çö‰^¸ó@ц B« ¿ÊnЖ
¦¿áÔÇq\þM¿×'r%-ÙO¿î.
)y¡PSRpsrPSR J2017-16?¶øZÕ	­y?¶ÓÌéSú?í ô¥^ÊR?¶ÓÌéSú?ÙN¶Ž?Òk¨"'‹?ãXÀ}x¤º?Òk¨"'‹?ÒpKEœ/‰?·oËÙÅ?æÇÚ]1è<?·oËÙÄ?Øá9/E?»;ÒÅ6–?ã7ãvè^?»;ÒÅ6–3FGL J2018.5+3851@S%öà1-Ÿ?úžÂÊ £À8­°"—©ÕÀ:'õ}Åþ?éfÛ+_T@â»Z^›A@Ô6€šš ?ï·¸ˆ¿æø…cF¿ç{g;§¿×}–³é°AGNbcuTXS 2016+386?ä÷Â19B?ÌàÙ̔ÇY?Ö{睍{?ÌàÙ̔ÇY?äÜњýÉã?Óf]R<ú?ÖF\Êl:?Óf]R<ú?àF'¸
?¾p¬J
ýu?ßÃrÛúì?¾p¬J
ýu?é;S»Ä'?»à
ÚRå?˱í÷ò?»à
ÚRå3FGL J2021.1+3651@RÎè_ÐJ0?¼éóŸÛŽBÀ5hÀwSôtÀ9Þè¬&d@ŒN¸@ý{|@ÛnÚ~;D¿ÕT.wÙø§¿á"~ièQ
¿æ¤7HÛTê¿íCÜq8/$PSRPSRPSR J2021+3651?#Þ9+ºœz?5'®`¦?ïþÂmDW?5'®`¦? î>ÒkQB?@Qjtï…?ïþñÙL?@Qjtï"?vօH×CL?qo[l7??ïÒRõnQy?qo[l74>ԃ>«ßÌ>Ü-´^;""?ïÿõ¾p`«>Ü-´^;""3FGL J2021.5+4026@SŽÔ2Tç@ªJ_ʕæÀ4Øï;Œž	À9҇'§
ö@K§ÍäÏÎ@>=@§:@¨[—ÖK¿Ók›
På:¿â*›Ö¤¿ç­»I–¾¿î9ïxPý&PSRPSRLAT PSR J2021+4026?ÈæÈÝ炞?ÎU›iì?éÆMȆY?ÎU›iê?Lú\»?z°½ú‰f?ïøÁ~ß»©?z°½ú‰f?ÓD
°.»Â?Ï !Åþ›+?æ]ù'è¢?Ï !Åþ›+?uêwZ*?Á®§¢?ïÿ®(W¢#?Á®§¢3FGL J2021.9+0630@HÐu@ýAÀ0ÅM¿¦sÀ9ªwhiÏÀ;m
[£"Å¿û»T­~«@
5#·j:@s\ <`ƒ¿àJ"+y3¿à`™. 
¿á‰ûcZ¿èø°1ze;AGNbll87GB 201926.8+061922?îÞS"Kò?¢Ee3?¢*ÍÛ@á?¢Ee3?ï¶ÍóGÇ?‹m·i=·æ?'L¾C.:?‹m·i=·å?ìck€,:ò?¬1O—€
x?¼ä£þž(m?¬1O—€
y?ïúÜډÃà?M2$PŠIX?DŒ•Øð"¤?M2$PŠIV3FGL J2022.2+3840@S6¸!ï?îÍÁ¿Ü&À7û_)[CÀ:G$ãW²@Óï` ~»@
e•ÙE¬@xH-Á.^¿ÝÐdÜÎw¿è‰œ*Œñ¿ë.P«>¡¿ïÿ†ÈÜ}DOTHERspp
?ƒ%Ä +¿?˜ë–~rÁ?ï³hïßQ?˜ë–~rÁ?)¶§¶B
º?D¨êU`}?ïþd•"›ß?D¨êU`}?¿Î#¼/?°_å+-C?ì;Ÿè|ú?°_å+-C?AžLùh?7̲D&?ïû¼Øl߁?7̲D&3FGL J2022.2-4515@v.F_•'ÍÀA:2 f<uÀ9°Ö?<VÀ;»>©ˆúæ?Õjˆ6<I@˜þi'@ÄAÿÿª¿áq—->㧿åõ7¿ßÔf¿æ‹"\!¿¿å³N÷^òAGNbllPMN J2022-4513?ï÷tNF‰%?Uäÿ`Ìã?Qcrí¶2?Uäÿ`Ìî?ï™Vw@\_?—ɽXat?‰ªb/èè?—ɽXat?îÍα	ý6?˜åàÁòã?£#ï`,ˆ?˜åàÁòá?í}#q¡`[?¢+´z؂¸?´ärôý/?¢+´z؂¸3FGL J2022.5+7612@[Sc€ß@5#ô™=SÀ8߃'gMÀ;€Å¤º_¿¸AÅ(£@Ëbôkø!@ÍÄÀcÝË¿æ|V'0¿äs ¾¦ïC¿äYž¿ʵ¿æX
6n|AGNbllS5 2023+760?ïò6¬‹¥s?`Й5LÙ?['¦èµq?`Й5LÓ?ïeFƒ!´ä?–õØEFÙ?"W/›ÉcŒ?–õØEFÙ?ï1	GÇ?g?"FöÙևù?™Þ×h?"FöÙևû?îú8®h5?":@|ĉ? \~¥|¸?":@|ĉ3FGL J2023.2+3154@QÙÜßÔçNÀ']ßYAeÀ9nwºKÀÉÀ;6jö ?ëÐ^_0çÿ@ çiõ@'x z´Q?ížf5F¼[¿ ;'Z鎿ãZsæŠA¿áIÑJ¾rËAGNbcu4C +31.56?ït±Í¯»?—u
<¨?'iÆ^Š¥?—u
<¦?ívƶˆZT?¿;¨-þŠ?´IÊK½-]?¿;¨-þŠ?íŽÂª_^?¢aBžqð??³‰ê­E?¢aBžqð=?ì•5§"lN?©Ìÿ¼'es?»VRÃ\Œ?©Ìÿ¼'es3FGL J2023.6-1139@@O¢ŸÒ˜¿À9®â_ܪÀ9'`uÖFÀ;T3—Ac?ò´bÞ©ª@µL¨z2?ÿV´öí?¦,EG ¿­¿ÚZ"|<ø•¿ÙÆ»®ÊáÄ¿çz8B'ŸûAGNfsrqPMN J2023-1140?íƒ^@梡?³çë¿íJ?³å
øÊêü?³çë¿íJ?íʋÎáiÅ?µ…|ÄÞâf?±«¡ˆô±à?µ…|ÄÞâf?è8%#çô6?´3§:Mm6?Ïkp`/*?´3§:Mm6?ç-14ø?«Köʝº?ÑÓ¥Ñ–?«Köʝ¹3FGL J2024.4-0848@AƔÿÖåUÀ8££Àd¾À9¹Í°!›[À;[Ö¥"¢à¿Ð&m2ï|¶@—pÛà;?û=ßÿ¯x(?ìñÐÖi%¿Þßo1CD¿Ù^ß§¿È°ÂHB®AGNbcu1RXS J202428.9-084810?ïý[
¾`-?8³Ãk÷?5'ªþ˜S?8³Ãk÷!?ïã7pd™4?tû¸âÈ#?lȏ›fÌ ?tû¸âÈ#?ï­L]â¼?'°ÌEiì&?"¬øè‡P™?'°ÌEiì%?ïüÞ!= ?<àL+Ȉ??qöû-?<àL+Èˋ3FGL J2024.4-3254@#>óà¿À@n¦`QyoÀ9<ÚvÙ{1À;@#¾†À°×º'‹Ù@å5O?b@OêÀ'ÍÏ¿éÄ:ê.)¿çØ
Ù¤¿âÉ	7¥ø¿ï¢3äÔAGNfsrqPKS 2021-330?ïþfAÛ_?/#õ®<P?)›ïòJ«?/#õ®<B?ïï!^–ñ?o'`ÖÄ Ò?`Þ¡iê"?o'`ÖÄ Ú?ïp÷k­Ç?ŽÑ~ÖíÐH?'áŽ
G?ŽÑ~ÖíÐB?ïÿôPrе>ç0Þo@>×_^˜/¸>ç0ÞoK
3FGL J2025.2+3340@RF–àU­ÀOÖOÀ7é£?4É5À:^zb?øÐ{ùF@…'Ԇª@ئ²†Ði¿â±Àç]¿¿éŠù‡"³¿æ"@¢Ã ¿íÍVœ2¿àAGNbcuB2 2023+33?ìqgOò͸?¸ò	yMr?¼tŀi'??¸ò	yMq?ì›\»Tof?Åûl•ö?»%%\"Ê?Åûl•ö?èV\£½Š?²Ã@ۗK›?֍sÁ	Õ?²Ã@ۗK›?î°å=&
'?žÝeÃ'›Ÿ?¤ñ¬-ŸVç?žÝeÃ'›Ÿ3FGL J2025.6-0736@Br® 9[kÀ8d:ঞeÀ7Wm¯0ÔÀ:æX"»@ܺ«@7ï<ä7@xãPÇÄ¿ßRáù§u¿å¥¨×¶F	¿æä¦É¿ëÁuuoe5AGNfsrqPKS 2023-07?ÿ"'?ŒÒ
T¿?\8Zە?ŒÒ
T¿
?ïã'h(`ú?y‡—Ó¢	´?l}—ןü?y‡—Ó¢	³?ëՏ…E[?¬Þ¨17m?ü©Áêê•?¬Þ¨17k?ïþmØ´9A?1룼ìÛ?)"t¼kÙÚ?1룼ìÚí3FGL J2026.3+7644@[z°<«'@54·¿õMõÀ:"TÊÀ;ÐóöÝA¿ò²cЦ÷@·…:<ý?ým8ÎAl?ì™Nw©§%¿½†"¯¿ÜÞj)К¿éäÁªÒ'AGNbcu1RXS J202633.4+764432?旅ž¶â?ŒÅ =‰´Ø?†_RGy?ŒÅ =‰´×?ïD@ÍÀ?«%Ø-ƒ
½?—|í÷æH?«%Ø-ƒ
½?êý¸ð™è­?±Xò×>ù?Ä	=˜]N?±Xò×>ù?ïØ,Üß"?}ÇáÕà•D?s÷i'n>?}ÇáÕà•F3FGL J2028.3+3332@RW€dÀ	¾ÀD©'À7xrϏÀ:pŠ)º
­@VVù¶æ@}$îÌÑÕ?ü£_9M¿²²U/åÔc¿Ú³íéä¿çýuûÉ~¿î:öå¥PSRPSRLAT PSR J2028+3332?-6Ï=>%^?'ž:þ|Ê0?ïþ,",?'ž:þ|Ê0?8 »pQ?LØ "­?ïüëèŽý?LØ "­?u³õ'#´c?px'Ö%?ïԘ±¸˜?px'Ö1?Au""˜Rð?5ÚEO˜	N?ïû¢žÛê?5ÚEO˜	N3FGL J2029.4+4923@U˜WŸúë@Z
@JÈÑÀ8rÞN«_À:úō=jÅ?óÁz´&8@o*s*©@I:ÀETô¿â½'ö{-.¿àb|>Œ¿égóI8X6¿ì
GÃ^vAGNbllMG4 J202932+4925?ç˜0!kV)?Á;Ží?Ðϟ½)S¬?Á;Ží?ï)xð…W?¬Þz†:ç?šÐáÿoU?¬Þz†:ç?ær©¸œöÐ?´§t‡'Ù?Ó¬ŽÆ`?´§t‡'Ù?í#F€Ð½?¡½º‡j?¶çÅËùz?¡½º‡i3FGL J2030.0+3642@S~ +ïr¿öçÇ¿Ç«¦À7΋ýϤÀ:ž;aÕÝî@øByw:I@ړ‰à?ø»B¶³Ûº?³ðïèkõÙ¿Ø_ÄŠŠ¿å«Lh¨#å¿î"¨FNPSRPSRPSR J2030+3641?#l¤€gáx? Rp'À…¬?ïþÉ5·ùƒ? Rp'À…¬?!Ñ¡%³õ|?>87´¦~æ?ïþâåí¤À?>87´¦~æ?zE2õÖ?yîÁðð£R?ïËuõ÷š?yîÁðð£V?"'£¶Òj¾?2}?X?ïþÖÕĒÛ?2}?X3FGL J2030.2-0622@CUv?ø="À8Û[¿CwNÀ9C†åaïÀ;[?ep!?ÈýWlÈÎ@'5·œäÓ@ 6à'Т¿èOÂ)I"7¿éPH÷Y'¿âj˜2CýŽ¿äòŒ~ËY}AGNfsrqTXS 2027-065?ïÿêP¤)¥>æuÚEtå>å¯[Ö[[»>æuÚEu>?ïãêòZ'O?x¥Þ%!®«?l
¥}°å?x¥Þ%!®¨?ïм¯6ãb?z'¯²|?w¡¨dŽN<?z'¯²|"?ïý¸h—ù ?(,WãÑGO?2<»@38?(,WãÑGe3FGL J2030.8+4416@T–Z?çvœ@ößoçšÀ7«ö©?)À:|^ʐ²j@©'¿šÃ@ã$ð_?ûé/Ï%—"¿Ôd=eÕ፿â
ñ!bGÀ¿èa9çéo¿ï·},¦|+PSRPSRLAT PSR J2030+4415?1ž;l½ˆ?*e$Ê	?ïýÌ-ø'i?*e$Ê?EB¶P›?TgJãí˜@?ïú¯RkÙ!?TgJãí˜@?t9˜2<J?^nè,]?ï×Ōϛ†?^nè,P?+»œE'ìA?#îA|*â?ïþDF;§Ò?#îA|*á3FGL J2031.0+1937@O( 2:À'`ÿX±À9¯˜JAÀ;o7…¨K?僧GŠ·@ÇJ	
šÈ?ý5ëˆ"¿ÛãÅñ«_¿©;!ØܔZ¿Øð8^¡`¿Ú·Ñ‰[D0AGNbcuRX J2030.8+1935?良€‰OU?‰^y¡3ÇÅ?†ßݬ*½?‰^y¡3ÇÇ?ïÆ%Ò*ý?¥FGG»Ól?ŸÇ;Eº t?¥FGG»Óm?îìXóóò?•f@ÄO˓?¡:pÎpÀË?•f@ÄO˒?îkdÓpqO?'2«LÝ?©I²Èøë?'2«LÝ3FGL J2031.8+1223@LÈ bÀ/mÇÀ'áÀ9Kƒg(-FÀ;4ÎAAð?Ô¥}}a@§ÃþÇò@yF÷¶¿ãQßy¹Õ¿åŧ(Zà¿é\1'&ç(¿ÝôÌõUpåAGNbllPKS 2029+121?ïî·gy?f&)'` È?aH˜å†æÝ?f&)'` Á?ï´êRé?Ž)*󛕆?'Åk|E¾¹?Ž)*󛕇?ï¯=óø?•±U¬ësÒ?œêA ß?•±U¬ësÐ?ïm'ø?ƒyª3'Êt?']­ ö?ƒyª3'Êu3FGL J2032.2+4126@T
ýòÿf?ðMô·ÍÀ6'•¿†À:ª¡(Ú@ðzú;J@
*÷%æÄp?ü†!'Kòr¿¿KŸ:ÃJm¿Ù¢#ÏN¿âmA'3ÿê¿ìY!d(ÉxPSRPSRLAT PSR J2032+4127?2#n_ÚKï?*`ú¦A"?ïý»'4¸?*`ú¦A"?%1PvtA?BÁþ'EC?ïþ¬îêø™?BÁþ'EC?u×ÃkEàj?mn™«&s?ïÔPy)tA?mn™«&M?àËÌٛn?õúu©ÓA?ïÿ@ù¡™2?õúu©ÓA3FGL J2033.6+6309@XŠ?ÿÊP@*þJ`vb]À:k£¢1ÐÀ;Ä×09¿"Þ#õ‰¢@C@1"J?þRa~Ë-¿êÌÀl¹‰¿æ"Û|	ˆ6?–Š-júÓ¿ÖŸjO:aAGNbcu87GB 203249.5+625814?ïý·ïECQ?1‡P.Nâ?2@…Õåxº?1‡P.NÐ?ïҞ J\?ÕúñÕ?v°ïûÚѹ?ÕúñÖ?ïÂkµÄä?{³QäRé?~Ê%ýB?{³QäRê?ïÙל?p^Kî$˜ª?sxw±÷[?p^Kî$˜§3FGL J2034.3+1155@L?› 'À0|rŸYÌûÀ9±vfŽªRÀ;wœÏÛ?åŽJݍ©@ÅÆ"8@̵ `]8¿åq¸ÆýÍB¿èÍò¢Ûré¿æ÷£"Šú¿å†>•^mìAGNfsrqTXS 2032+117?ïåã|'è"?skWRº¢?jƒØ{x?skWRº¡?ï¬Ä®Õm?'Šþú{?"ÎÔJ¤¾H?'Šþú{?îD°ý¸l\?¡êõ$^?«´ð$y:7?¡êõ$^?î¡õcÐo?—hGà=€?¥à©Âÿ9?—hGà=€3FGL J2035.3+1055@K°‹ßœ³*À1;`c'À8ihÎör¹À;'ÃbÀ¿x?óÉ®	h4@¼0V½@¾4à1ƒ†¿á'Zr^¹–¿æ†?"ë_	¿æ´KÀÈ¿êAë1^>FAGNfsrqPKS 2032+107?ïñ×E|Y?Wv¥õq£??\QÃuN3?Wv¥õq£5?ï¹L¨¼‡÷?‹0Oí-Ä1?¬ÕÐÞ	?‹0Oí-Ä1?îS|%ù?œE|©þÌ?ªÈ>­ q?œE|©þÌ?ï¦:c;W?x@A(.Gˆ?†±g1*‰?x@A(.G‰3FGL J2036.4+6551@Y(¯ ê[S@-ÒA³ÿÀ9¶ñµºaÀ;¦‡dã¯?âG»){_@¯^ìI"É@€-?¿áDˆ¢V=¿à¢8±ø50¿Ó¦ã¬ë¹€¿å‰_ț|AGNbll87GB 203539.4+654245?ïâø5¦ËÓ?pRHx™89?mÊY4-Œ?pRHx™8<?ï"_Æ¢`?"jØ©ªû;?‹(<ÎWh?"jØ©ªû:?ïjz½·%?C·E£?'°¨I\$?C·E£ ?îs/€
þ3?–ÈWF"Ú?¨Íÿ ¼?–ÈWF"Ú3FGL J2036.6-3325@#X+€~
ÀA½â:¸cÀ:žƒujæ(À;£Ýs
=Ö?æז(î-<@
–B	òa?ôàÓËr/?íš|˜ì¿ïïrȖÕ?ï¸t´™
?×K;IÕAGNbcu1RXS J203650.9-332817?ïü:Õ·T?H éËîQK?>)RGU?H éËîQ%?ïïVʃª?i«Ú=ƒ­ß?`©ñ5|V?i«Ú=ƒ­ç?î¯øÏöÑ?›
§[.w?¥sŸÒñ?›
§[.u?ïüŸ¯µUÁ?SY–'BÝ`?;'UQôû?SY–'BÝ`3FGL J2036.8-2830@/Êœ£9ÀA2¶­À9·'%VўÀ;ªÀ:ñiš`>F@í-–¼¡@ž˜›ü ¿â´låö-]¿å¥F‰Yä¿çÞùÎ@G÷¿çe±jFAGNfsrqPMN J2036-2830?ïþ½€"y]?"™‡Y°Í?$'ýØjBR?"™‡Y°`?ïì>‰)>?n—¨YÄ ?cÁ÷vÖÁ¦?n—¨YÄ ?ï®_c™Ó?ÆgDi?"h:§‹=?ÆgDk?ïú7JŠ2?FD¯÷*Ñ?G"Õ×Ç9K?FD¯÷*×3FGL J2038.8+5113@V/×,uª@Ò½ßôò±À8˜ÈQ=	vÀ:¯ÚM¾Ð¿ü"ƒèØF@ŠÆóïÑ_@!ÙŒÂÇ¿è~3•6f!¿êö°Šï);¿èó"ëxš­¿ç·Õˆ¡éAGNfsrq3C 418?ïû@Ö®ƒ?GÞ¢Á¤÷?Bü¥GõùY?GÞ¢Á¤Í?ïÈ҇1¨H?'À6©e?{–¼g+Ûì?'À6©d?î&·¦óV¸?£Èø.Â?­"…Ê"Ÿ?£Èø.Â?ïÿÉV—ç_?÷"`Ží>ûT´Q6Û?÷"`Ž:3FGL J2039.0-1047@A£Rÿ" À<½ÜŸ¨§TÀ8¼äÏøÑ8À;8E­‰:§?÷8(Øîn@£$¨«Û;?ù§´³Pz?§†õŸv¿à:3Ïݛ¿â}zvÒ¿â7è6;6AGNbllTXS 2036-109?ïõ"5¶ÏT?aÔÒa÷X;?U»"'aW©?aÔÒa÷XA?ïpÒâíÁ?²êIxF?Ÿ壢G´?²êIxF?ìÂòwi??ªµîV–ò?¹èlD·½û?ªµîV–ñ?ée
˜yJØ?²yÜ®êN8?Êk՞ԟ?²yÜ®êN83FGL J2039.5+5217@VkΠ£¢@
æO†%À:'r—ÍÀ;_®FÏÈ*À7Õñ
ÉÂ@
Z×h\4ß?þGàðñ?ÜMâ'QåŒ?ëHo«¿âP¸S¿Õ¦Ð†73•AGNbll1ES 2037+521?ïï±õS—ë?_0y"!~>?`N
¬hM?_0y"!~6?ïÇ4yJH^?À"@©^?|eÃZÛÐ?À"@©_?ï"âêG?{æ…0=7?›£§j·?{æ…0=8?ïÿ÷Èàa‡>åEvcК>Ðn?<õ•w>åEvcÎ)3FGL J2040.0-5734@u:jŸ{ZêÀB‡ŽèӔÀ:O»¢çÀ;¹Åԋ0¿þî5'³÷>@
ú…\ '@'Ñ`w‰?휃OÄþ¿éó£ËC,G¿Ö[âé2¢Ù¿ìK%99KjAGNbcuPKS 2036-577?ïó ³Ôè"?…ÀÛé®?Y¾˜V/¹à?…ÀÛé­?ïî'[Y­?i—§Ö³?am¤¦Rýo?i—§Ö¸?í†"z?¢=4íHvÈ?´Ëß'd)?¢=4íHvÉ?ïÿƒ¸ºEì?]Vȇ?Ñn…!?]Vȇ£3FGL J2040.2-7115@t2gŸì™òÀAá`xÀ9§™hò1áÀ;†‰1l‰–¿×ñÆ<Ÿ@
Õc¥ì¹&?üÃöM½ù¿æÔcGß"÷¿ÕŸ–äL_¿Ö˜÷f7±¿ÑèP©ï/×AGNbcuPKS 2035-714?ïû¾Ý«½þ?A=ýȤ%?A‰Q	?A=ýȤ=?ïé©3‹??pdU•2
^?fåVÌtÁ°?pdU•2
a?ï¢1r6k?§Ûr¸ò?‡s¸£rdó?§Ûr¸ñ?ïã™äĤ4?f¡2~¯Ú?lf;[Ìn?f¡2~¯Ú3FGL J2041.7-3732@gE_ۇÑÀBš$€	À:w$ú‹LÀ;—œ`ô6ž¿æ«ªùÆÞ@
¹« éð?ü™Þ¸Ý'?ãà¶cÁ¿â·£??¿ä\ÓÚL¿ªwYƒAGNbllNVSS J204150-373341?ïúµÚ?k?K'ŒŽ#©?E(—TÙ?K'ŒŽ#Í?ïðñK.G?gștðÖ?^iÏ£r?gștðÔ?ïô6Ï]¶?•NèZ¨?œáy&Ia?•NèZ¦?ïûÛ#²s¯?@)ë;eÿ?@"q61Gø?@)ë;eû3FGL J2041.9-7318@t
ÀÓgÀ@Ýn˜K¼À:¬(©lÀ;ɨÛUüŒ?óVµ"ö@Ë$Np@­œ€~Àz¿é«-ˆ×Þ¿ëM‡sb‰s?»fpѓð¿âw ‰s—ãAGNbcuSUMSS J204201-731911?ïõ5ÙpG?a™¹fžÉ?U"MÍpý?a™¹fžÉ?ïÏcd4m?"Ð6Oëü¤?xuÎMåÉÙ?"Ð6Oëü£?ìrA‰'»¼?©ûÆÄB¤P?¼mó¶Â" ?©ûÆÄB¤R?îpÃ'OZ?ª»åî9?¨ó͋šm?ª»åî93FGL J2042.1+2428@PòaßîèÀ%–Ä!, rÀ9ÓpàÓÀ;†3çÀ½¡7Ì¿@Šþ@8ã?ýß#ÿŽ–¿ëi*Ý4Š2¿Í'«é[Š¿Ôjë%¨[(¿Øb' 4AGNbllMG2 J204208+2426?ïýyþ8¹~?0npö8L?40:4}?0npö8#?﹕F	Ñ?"2å«zÂ?š®}‹¼º?"2å«zÂ?ïÔE{u'Â?r In¬€ð?uÝBEl	?r In¬€õ?ïÿýS?x>Λ¬Siƒ>µf;ç5>Λ¬Si‹3FGL J2042.1+0247@H?÷fÔÀ6ÿ n4'À:Y)ªIëÀ<:&1Âð«?ù)Õq6#(@
É, ð:?áçy©í­¿ËZfØ1¿Õ!÷'"b·¿îOÙGÀš ¿ßk;Õ:¦çPSRPSRPSR J2042+0246?Ûz%nUÔô?Õß\4—?âBíHÕ†?Õß\4—?»ûˆ'Óº=?ËLÓ—
?쀎ûˆ¸?ËLÓ—
?ãD|î¼?¶š,Û©?ÙwÆ"‡Õ?¶š,Û¨?š¬M—¼Æ¤?©HsJ«ë?ï*"BÌ?©HsJ«ê3FGL J2043.2+1711@NóK 'ßÀ.šDÀú0³À88í¥,uÀ;I»	Uê@¦óp.@Q	@¢C@Èx»¨'¿×܀"'(}¿Ýk'oŸcø¿à«ƒ½u}¿ì«Àã†PSRPSRPSR J2043+1711?sø5¤…X/?oi¢O^œƒ?ïØ"¶õN?oi¢O^œ"?"ô!l÷õ?š|JK@?ï¹ì/zL ?š|JKA?'²bÇ%?ŽWíÅTÈ?ïrléÆ×À?ŽWíÅTÒ?‹y'U¦ë?%éäÀS¨?ö©e?%éäÀS¨3FGL J2043.8+2741@Q¨¸!ïÀ"NîÀ¨tÀ9*AÖd%DÀ;ré?û1Œ$;¸@dóiï‡ã@4J´RE¿Ö…<6ß\"¿àú¼Ê J¿êia@óÌQ¿îÚâvy¦WPSRPSRPSR J2043+2740?Bò|FCgP?>‰²Þöo"?ïûC`îo&?>‰²Þöo"?j½Þå:¯@?s¾ÄÔúþ?ïåB!ÅR?s¾ÄÔúþ?Œó#ק¹?'5®·ò?3p¡a?'5®·ò!?'ð¯ˆQÿ\?y:¼ùn\?ïpzƒ½p?y:¼ùn[3FGL J2045.2+5026e@V06â—@®k³¤ˆÀ7"S‹˜OÀ:C/(·Ä@¢ó_2•@G™E`Ý;?ýÆøÒ¿Ï©0&Ž¿äùÄ÷k¿èƱ?R¦@¿ìÃ"Ê/c›OTHERSNRHB21?`M7¥™?aÀÅv¥=?ïï²ÈbZà?aÀÅv¥=?`þâÛNžu?qyu±ö"?ïï$±a?qyu±ö"?Ÿí"€?Ûb¦QN?ïß "Ùì?Ûb¦QO?Tè'M h¡?Mz'F'?ïõ‹¾ÙoÌ?Mz'F'3FGL J2046.7-1011@Bl@%NÀ>2w"^À:jSâÖ#ŽÀ;"bۗjë?À'@"ɝ@ŒV¹ E?ù¿WAï9?ïðª(¡Î‹¿¾½mÍx¿×."Â3/œ¿Ï$ô'IÕAGNbcuPMN J2046-1010?ïý­ëÍÌü?1ыk}1?2¡'˜({?1ыk}o?ïå½yŠõx?sÎÒ j%?jB†u
ˆT?sÎÒ j&?ñ?µë¡ë?‰Ûƒ¿<?a?µë¡ë?ï˨¿ýJš?n }aúkZ?z+ Z³?n }aúk_3FGL J2047.1+1054@Lˆ)³únÀ3¦Ÿä6vÀ:\l6‰ÿÉÀ<,)ñk?øyȈÅ`ó@-zØcXë?æʒéYÔ?îËa¦Üi?ÄOð Âv¿à"¥…¾¤¿í¶™£ÄY¥PSRPSRPSR J2047+1053?˜¡‡âË®?´Žî5¬yG?ï:óÀéã¥?´Žî5¬yF?Àð41?ÍîÁúáç
?ëþþ²ó¹?ÍîÁúáç
?½«ÎŸqh?·W2>þÚÍ?ìJ†,Òü?·W2>þÚÍ?ћåpᜄ?½ÿcf\€;?ç2
G1¾?½ÿcf\€;3FGL J2049.0-6801@tj‹@p2˜ÀAò¨`úÀ:%êIµU¸À;Ä)Ĩb?åæ)Aí¶&@!Úi˜u@xÓ@Yap¿íƒ˜í»ô|?ÐìMë	<®¿â§ým‡¢¿åGqaIÐAGNbcuPKS 2043-682?ïô
—‡…?`oŒP5w?WêÑØðô?`oŒP5w?ï|Fp°ÚÊ?˜Íþ¸RE?w1é䦘?˜Íþ¸RE?ï6Fm¤©½?‡uWUg8?™72KjÈ{?‡uWUg6?ëëÝYš™?«îƤæe??ÀPŠ›…•?«îƤæe?3FGL J2049.7+1002@LWú€d>nÀ4­€'ÍÀ9=A&QÀ;|v,­5?ÔSÑA@j•pj @9Ûm¿å\'"Á¿æÑX«Eq¿åÇiX¿ç‡ëÕ·¾.AGNbcuPKS 2047+098?ïôì°P?gŸ€•>š±?Wö'îŸ^Ô?gŸ€•>š±?ï­¬[|?'¼r]s?""üi ù+?'¼r]s?QM§w?ˆg_ñ N?Œ«¬–",?ˆg_ñ M?ïWå™CD?"Í:ob?•Lחx?"Í:od3FGL J2050.2+0409@I·PÿÌÔZÀ8t-݉À9Ø
¨_/À;"8PÍx?ã<ð×v§…@
$*ÌÝ=Þ@‰¨f翕ЉÍô•¿à4Õóo¬i¿ÝmyzÀ:˜¿æÈŒ·€WAGNbllPKS 2047+039?î˜Ú¿oJ©?ªÈ[Ûé}ó?¦rT	U}?ªÈ[Ûé}ó?íÂF¡C¬æ?²°eø$#í?±íÊõâ˜Ô?²°eø$#î?î ºeêÄ?£ÁE["¸M?¯=ôY¡S¿?£ÁE["¸M?藴ˆiP!?§¹M)O*?Í¡-ÞZ¿}?§¹M)O)3FGL J2051.0+3040e@R¿íÁ9À! ÀŠÀ78IqcÀ:ŠÂp@°1a÷ÁÃ@òäñܦµ?ýÜSûª°Ã¿Ðþ¯¾3G¿ãlˆÌ¼¿åSºÇ犾¿ëÈeÊ_4COTHERSNRCygnus Loop?Vw&‰cÝ?S1"4X?ïôÄl»Nx?S1"4X?Rä¢Õ÷Ç*?e"ÕšßP?ïö®•?e"ÕšßP?"UüMX`?"çš–+¿?ï]P•?-?"çš–+Á?bÝ54?W.N/†¢y?ïí"ÊóñÍ?W.N/†¢x3FGL J2051.3-0828@C™* dúVÀ>v |wJÀ:yö£•œÀ<FÁƒÃn?ú7¸ék@Ë»O†¦?æ¨Ì]Ÿ÷?ïÿœ)''?ÅýíÍž¿ã4Ìå^¿ïÿMfÿØ,PSRPSRPSR J2051-0827?Ò{Í<ºuX?ÒJ²UÞ9?æÂa¢ÅT?ÒJ²UÞ9?«Â—ø?Â_ª8¹	?îCÞö€~à?Â_ª8¹
?ÌOµµ
ÁK?··ÒŒJ?èì'¼®?··ÒŒJ?¸¤;š
‹?±1æSف?ìëxœ¬¾¯?±1æSف3FGL J2051.8-5535@u]Ø`fÀCx) zbÀ9ÔûÔ!TäÀ;¥°a\;j?ÇÞ¼Eb'#@ã'ÎQ@ž^ qº'¿ë ™¸Md¿çúË¥ÕE¿ÜqtAEo¡¿àGŒ5zW¬AGNbcuPMN J2052-5533?ïÿçù0a´>ëÔæ"ôÓ@>èϞK5ñ>ëÔæ"ôÕé?ïðêpѨ?eíìG•ãÛ?_ò+\²S?eíìG•ãØ?ïß̳­ÍA?uÛ¤Onö*?p¦)_@?uÛ¤Onö)?ïô 'ː?K™ÁUŽ{d?V¿°iÜÝQ?K™ÁUŽ{i3FGL J2052.7+1217@MŽnß±«ßÀ4ù@ÉìÀ9Á+KÞ$äÀ;˜†1		?Þ"ɘ\O@
TŸãŠ©@¿ÑÔ¿àÍNnðE¿ãQ'KŸ:ÿå4'౟ä¿äùÿäþ›PSRpsrPSR J2052+12?îÝTû¾?©Ö‹6ÅâK?¢*°DM?©Ö‹6ÅâL?í÷mP'"?ÀBùë|ž?°D•Ûîä?ÀBùë|ž?îgeӗ•?Ÿé'Sðr?©‰¢Æ†¯?Ÿé'Sðp?ç©]¦\WÞ?¶?ÍK|'F?ЭD³GPD?¶?ÍK|'F3FGL J2055.0+0016@H9Ÿ C×ÆÀ;
v_Ø­¬À:xÊ J"cÀ;ž‰.‹C?)ÃZ<¤c@úׯ~Þ,?ûºb&%Ú?ïô>!gž¿èþúÔÇíë¿Ú°à¤a
¿›K§7µ"AGNbllRGB J2054+002?ïÿkC é?&§£•bDÜ?²—‹ãó?&§£•bDõ?ïçÂH¡/?r%_|–™?hà=·^ÐÖ?r%_|–™?ï­°lND?~¤*Ž=Œ?""þ¤ìnß?~¤*Ž=x?ïíæ¶.jº?[ã€p"c?bIѕE?[ã€p"c3FGL J2055.2-0019@Gó¢`¸À;hT`ªdÃÀ9ïtŠ˜À;cÌütð?Ü —8°•@hcJ?ùÿ!@AŽ–?o=òÌ¿¸íý^C¿Ì®ÅG>пÓm•¿ÅRZAGNbll1RXS J205528.2-002123?ïåZêܾ¯?q°ŽˆxI?j¥#AR?q°ŽˆxH?ïÚ;!Ž¥©?{!ï}[î?râo8­*Ì?{!ï}[ð?ïXê̑ ³?‹°:֘?"â¦mËé–?‹°:֞?ïš^<&–¾?€Mn¦ì?‰hpöZP€?€Mn¦ì3FGL J2055.8+2539@Q¬iöZeÀ)
¼ßÿ«À7 Ž]%uÀ;=¸·a+@~ÃS&m¨@JԏŽÔ?ûÄwÌk¿¶ÖĪ5ël¿ßc–éÍè¿éñ8‡¹zé¿ïÿÛrW
~PSRPSRLAT PSR J2055+2539?prÕd`Ø?xEø‹À?ïÞåU7??xEø‹À?WÛÄ1Å?dnP{Æ•?ïôsç?dnP{Æ"?žðyßÍÏ;?š/KÉ:{?ï|1'…?š/KÉ:y>÷lU#"¶>ûÆyóL˜ž?ïÿÑ'Uɸ>ûÆyóL˜3FGL J2056.2-4714@v	k¿×ÀD0½ßÉÿ"À7HErÐ×ôÀ;|ê6j?ûü%íûE±@2ê
$@©³ûo¢z¿áO,²]r¿æ㺠^Ö¿çºg΁"û¿è;¤=XóYAGNfsrqPKS 2052-47?ïõPÓ&²?Uë}ñ?U^YѲŸ$?Uë}ï?ïòkÔj4"?fN—?[XU?[(W+–ہ?fN—?[XN?îÉ/GwÑ?››¦WåNi?£mˆŽ²Þ?››¦WåNi?ïû…*æ¹?K%ƒ™ÐO"?CíëTe©?K%ƒ™ÐO3FGL J2056.7+4938@VSI`0Â@@ô´À;™ßÀ8ÖéÆ×qÀ:ågÉ<õT?é
"v"ÜÆ@[uLj'?üˆH€ø8¿×
Àي±†?ïýmaw¤¿×:CÀãϿݨSíN2ÏAGNbcuRGB J2056+496?îðúÄ	Ÿè?ž"•ÐsT? ðS¿fœ?ž"•ÐsT?æÊ'qw—?Ò¼èê4?Òk±ðÒ?Ò¼èê4?íÑëèRß?¡ñ'p2¸?±p ¿Mhý?¡ñ'p2¶?è‡ýå·?¾6dž"8?Ïõài(?¾6dž"83FGL J2102.3+4547@UÀÇä¡Ö¿à	'€4\˜À9N‡"žyÀ;˜áãµG?ù°Ñì~@¡/Æl5ˆ?÷Kc-vÛª?´  S¿ã¯¥$W¿î£#á[¥¿é¼å~tz%OTHERNOVV407 Cyg?ïB䙆¨? ´ ^´r?—£g¬Ï*þ? ´ ^´r?ç(QˆëtË?Óð_•q"?ѯ\î)j?Óð_•q…?æ2ï笂
?³JJØ¿?Ӛ 0¦ûì?³JJØ¿?ïEª¤‹…?—Vëaoíø?—\ª«nY?—Vëaoíø3FGL J2103.9-6233@tË¡ ÏÀC{+ŸÀûÀ8è_⾦™À;em¼Øc?é90&³Û@Y–ù+O?ÿ›I?2É?¯Lùû%¿â¥—\[(M¿ÞLYy1Þä¿ãEÊ/ŽŽAGNbcuPMN J2103-6232?ïþ,º«\s?,P®‡ú¶?-4UJ8êp?,P®‡úÞ?ïÕ¾çø»?{BA€ÔEØ?u Œ{ƒ¢›?{BA€ÔEÖ?ï–çJß[ù?ˆÐþiì?ŠF-H)ù?ˆÐþiî?üÕÍ?"­wdw‹?¦wð2£Ç)?"­wdw‹3FGL J2103.9-3546@aåéSÀD³, zûÀ9tÀ#i'À;§ò¼JžŠ¿Û÷øYÃjÎ@wçî@ç@GD¿ç	taÀ¿ä=t:ö‡¿ÛJÝQ‡å›¿ë²æë´×AGNbcuNVSS J210353-354620?ïûð¬½Ë˜?>Oê#ð?@=Mљ£?>Oê#ð?ïñ™0Â:¦?eЌ¼ÿ¦}?\͞{Š±‰?eЌ¼ÿ¦}?î"÷I"3¯?áÏÛ¤!Æ?¦°‹g¼Å&?áÏÛ¤!È?ïýû£Ú#?0<6ÒÌDm?3"á.Ûè?0<6ÒÌD|3FGL J2104.2-0211@G°l_¤«FÀ>Hï 6kÍÀ:­ƒðºèŸÀ;²/ãšj?èÄàåç·@$+"Ãyg?øbIÿ''ì¿î86#	ð?ï²ؖO?ª¶Í±ú
£¿Ê]JÚùòAGNbcuNVSS J210421-021239?ïöÅ_»?WUM"WWL?RÞuAöˆÝ?WUM"WWE?ïÌôà·n?"q±>ìd?y…þ¤Há?"q±>ìe?ï5ã—ŠÑ?ŽýM×­oâ?™C?ŽýM×­oà?îØî.hLÝ? ßtÝÑRê?¢q{2/? ßtÝÑRë3FGL J2106.1+2505@QðMÿÒ³—À-\n>¡ü?À:íA·ZuÀ;âž43?ØR‹!J—B@žo}¼Ch@8©€—j¿Ú‰`&x:¿ë9¤@^p¿éV/3¿Õ€ùŸ¾¡¼AGNbcuMG3 J210642+2501?ïªòÒã
?'Âe«G{?…CKG:ýy?'Âe«Gz?ï~¯-Žr?¢ã²¯/h?*N1¼°?¢ã²¯/h?ít‰¹µg?§Kî.‰(ž?´[²2W̾?§Kî.‰(ž?ï±)øÃa?"|gV•ê?ž)ÚÀç"Ú?"|gV•ê3FGL J2107.7-4822@uîâ@1HwÀEéÿãzŽÀ:Ú
'/ðÀ;ª¢år¶¿È¯!²x@d
"Íڔ@°vÿeÑ@¿êÎ+‡ ÑO¿ëyµbÛ¿Ûý裗õ*¿Öû%¢sTXAGNbcuPMN J2107-4827?ïÿÍ*ö®>þÍ^\834>ùpj"©o›>þÍ^\83£?ïñê["?f^ºÙ‰ÿ?\+Háî֊?f^ºÙ‰ÿš?ïÉëöðÄ?y'OϺ‡Â?{
x"‡®?y'OϺ‡Ë?ïïåû^ïð?Sëÿî¢j?`¡›?Sëÿî¢j3FGL J2108.0+3654@TF= ÿ:À،` &;À9ûì_9K{À;8Ò¯dÝ?Ú£D¤Zú@
ŒnPzÂ?þñæ­j1¿ì¯ižª%¿Ò
ØznÊÓ¿Ò8ÁS-4Ó¿Ýäî–VAGNbcuTXS 2106+367?ïñcÁjKò?TB.zÅl?]8}+hÎ?TB.zÅm?}?¸\°n~M?®~Ä68'?¸\°n~M?Gƒ,½?ƒº&ûkz?ŠP.4Ðí?ƒº&ûk~?ï>b
±`?‰í#"Ô­¡?œ3¾IÔ?‰í#"Ô­¡3FGL J2108.6-8619@s&¥?À	pÀ=)¿"å­À:¯º¨¦À;Õ"[tšÝ¿ë÷>$þ½
@|É®4[Q?û×à3¿Øm1Vd;¿è—t¡mN¿í§Ðë"6Ë?펨¬S|÷AGNbcu1RXS J210959.5-861853?ïîdÌkúÐ?o@úuÔ%®?a›3"/¿?o@úuÔ%²?ïèÜÁ™¸¼?pØ;è²n?g#>fGCƒ?pØ;è²s?íw"
	l›?¤£Ühë ?´C_—´›&?¤£Ühë!?ïÿXËø8®? ÒÒxZ?æ€øêœ? ÒÒxI3FGL J2108.6-0250@G±$€	À?"›Ÿ-WQÀ:6û>ÐÀ;á3}]?à{@,Ù@
¡nŠLI°?ÿz 'z?îÖî&
Û¶¿ÑùÚ*Èy¿Ý0°ä+Ž¿ßF³u/NoAGNbllTXS 2106-030?ïô]$½4"?\¿áŒà ?WE¶…–Ø×?\¿áŒà?ïÊZ¡¹^ÿ?‡°¼Îý ¾?zÒ¯#P€¥?‡°¼Îý ¾?ï5Èð?'""F{»?œ™Fþáî?'""F{¾?îeýJæÛ?žv.=™?© +Q'O?žv.=™3FGL J2109.1-6638@txYÀe¶=ÀC"ÿ®¡iÀ9‰³Ò*àÀ;ª'	±¿ÔZ䯘ñ@Ô×cL@´ 06ª¿æÀøùÙþ¿Ú"Îl›E¿â;ŒÊº¿à–j»­AGNbcuPKS 2104-668?ïý<:³ž›?Aø®‰?6*c)¥?Aø®‰	?ïè°{`í?pŒ´(†#?gO"Ÿ~?pŒ´(†#?ï'ÿÿÚÖ?ŠS~üìˆ~?@	O'?ŠS~üìˆ|?ïßµ³0?dî4lÃlÆ?p~¥&güÐ?dî4lÃl¿3FGL J2110.0+0812@Mş±áÀ9׊Ÿb0À9(µ)B©À;gS˜-ˆÏ?냚þRþ@3N5m=@š)€Výh¿ç˜õªf›j¿ß'<ä{®ç¿ãÐJÝ7ÂÔ¿ì†Ð¯ÝAGNfsrqPMN J2110+0810?í"¢oÛ?¯á÷È>7?³ßï/?¯á÷È>7?ïT="¯Èk?œ‰—¨ÉN ?•x[ªò~?œ‰—¨ÉNŸ?çܳ(*õ?²6•>™lC?ÐF™¯Íª?²6•>™lD?ìè
Ýh^5?œÁ/^¸@Ÿ?¸¿©½_?œÁ/^¸@Ÿ3FGL J2110.3-1013@Cè
`:Ó;ÀA·q?Þ<aÀ9™,å;XœÀ;˜£Wˆ}?íjìÖ±@íÌR(—@±íӄø¿âœJ–|-οì‹ßG<™¿ë,•yT¿ïö©¤2-AGNfsrqPKS 2107-105?íÝÕ`«Lˆ?±v¦ÝH?±Tú¥›¸?±v¦ÝH?ÞÖ–'Ÿâ?Еã	XxÁ?à"÷4·0?Еã	XxÁ?êè-9«ÿ?°ßQ÷w?Ä_K‰P?°ßQ÷x?Ë(Y0¸¾?¯Â¦zl×d?é5é³ÑûÑ?¯Â¦zl×d3FGL J2110.3+3540@Tå€!ùOÀ Éî E>À9­¸¨RšÀ;kŒñëjG?¨—VrxNŽ@çêô€@(WÀi ¿ä¼ó¢	æÅ¿åû§":´Ô¿èþ8
,Ñ¿ïÿv¥NAGNbcuB2 2107+35A?ï½G)҆?ˆ¼×'cýÎ?€ºn5‹^÷?ˆ¼×'cýÐ?é{°þRåH?Ì{³¸ß?Ê<´jÜ?Ì{³¸ß?íÜå	@Ç·?¢ï…eÚè?±×µùÂB?¢ï…eÚè?í_­Ñ†
ø?¤}°O¨ã?µ'sϐ<?¤}°O¨ã3FGL J2111.4+4605@Vy?ò^W¿÷v•âHŠÀ7ÙôŸy­kÀ:ÔàáVǍ@›}¸èi`@©€`7£@EÓ¿b:¿Ôqeóп۔Îs•ùÒ¿ä$Ä
'f¿éÖéë¸í"PSRPSRPSR J2111+4606?u¢ô!iz?z8>­C ?ïÔº½-
?z8>­C ?5¿¸‹¹˜Ó?W©¤þBÜ?ïýHîˆÌ?W©¤þBÜ?µÏõ-Y?°ñ~̾:?íFZ]œ–?°ñ~̾9?uàpœ\ÒÕ?j[VfB-,?ïÔ?ÇFZ?j[VfB-+3FGL J2112.7+0819@MZqÀ6¼UÀ:OoŸËÀ9‰˜ð&n)À;b8¤Œ;ã¿Á"^¡\@r¸¥š"?ü昛ü ?݋ë¨|'Õ¿ì®w/?j?Å¡(†Sc!¿Ýæ×½
3'AGNbcu1RXS J211242.5+081831?ïý׶X?7n­—îß?4GRM??7n­—îË?ïâYBĪ½?vµÍ]íG?m¦½;UBÑ?vµÍ]íG?ïš>¦î?"ÙªJWÎÄ?‰z°|ÖD®?"ÙªJWο?ïø^握?ROÑùœ?N‡´eÁ™?ROÑùœ3FGL J2114.7+3130@S¢åx•À'Äi¿·:"À9ÿôU§ÒBÀ;† Ô÷=º¿úÂc·àV—@Er•É«Z@ʺŸÎ'ô¿á?+¡Ä`m¿íñw³Y¢ø?Ù"V³¸¿ì¸ö´&ãšAGNbcuB2 2112+31?î•N"Ë0ç?´öšŸºÂþ?¦«ÓLñ?´öšŸºÂÿ?ï¿ß±	"?ŽGUÎ šF?€»½·w?ŽGUÎ šE?í"Ú]r?¥Øß*±^?¶é-Û|y?¥Øß*±^?ïþáTªµ?<àòJ†"?!îúµT­/?<àòJ†03FGL J2114.9+5448@WÁûbâ@'ßÕ=4À9Á¸øÚqÑÀ;ÉÜCbU`?ø½üë"£C@·\^¥§Å¿ùÄ™€í¿ÞYÀw÷)忲o¶*ÁA¿Øђ©æBë¿îiYÙÌJØPSRpsrPSR J2114+54?äÿ‡¿£n?ÛZÕë?ÖðÜ¹%?ÛZÕë?³I.G?ËXh
5uÊ?í–Ú?×>?ËXh
5uÊ?ÍA¢EAÊg?µÔ_P~i?诗n¯g?µÔ_P~j?«ßKx'?µ-™
˜V?îBHvç?µ-™
˜V3FGL J2115.4+2933@S'"Àh¡À*™egÊÀ8ÛN?(3üÀ;lw—|?áNø>ѳ"@ʱ…¶Ÿ@û
_d¦¿å•´|ôÈ>¿çæb3Ò¿àÔ¡Vì¿Ü]™j#AGNfsrqB2 2113+29?ïüç*?=ÓŽy§??ˆÇ÷Öµm?=ÓŽy·?ï†Dr»´?"ü,hôIÜ?ŽxnãQ÷?"ü,hôIÛ?ïS]Àüâ!?"&-³7¤´?•"Gàc»ñ?"&-³7¤µ?îê»Pœ£Ô? > !h?¡TJö5ÂÂ? > !i3FGL J2116.1+3339@Sóˆ` ÒÀ%K@¡À7ôò3Ž£À:Öøp¿…¼?êíª2‰b@AVóרž?þ"ëßâ~:¿Ù@Müì¿à‡Ùí`"ê¿Õßy¬X&÷¿àŸA=%êAGNbllB2 2114+33?ïûk¾?Dŗ%Bl¡?BRùÁE?Dŗ%Bl"?ï±Ì;þ<?'Y.ÙÐV?ƒŒñ}0õ?'Y.ÙÐW?ï–9ààËÜ?‡~ YV.?Šq‡ÇÍ	?‡~ YV,?ïòwR{Q?R^'4Ž7?[[	\Õ?R^'4Ž73FGL J2118.0-3241@(üT@Éô«ÀEó; g~"À:BÌ}À:æÈ~‰rÛ?ۊÒðÄ@
CùÂ#P'@|#ꬿè­Xíú;g¿è`"·"Ò¿àƒŠÚË#f¿Ùq·z!¦AGNbcuNVSS J211754-324326?ïö\‰*º?gšÆÔÚø?SFíª?gšÆÔÚò?ïòCíà?g4R4Ď	?[x%öàA?g4R4Ď?ìï¨1Ó?°vIžp7?¸'¾qãgk?°vIžp7?ï†Y'Õ?ˆØ	ã¨Á"?Žiœ»6
¦?ˆØ	ã¨Á"3FGL J2118.4+0013@Iû
ÿ±À@Œ@ÃÀ:Œ"\BööÀ;ÓáYKË°¿âM4CÝ@
Ž°?ÿ_@wÏ?4…¿è&Ÿ«Ÿ¿ØÀúýÈÔV¿Íô÷×E)]AGNfsrqPMN J2118+0013?ïÿßÀá1>öèˆp¢>ð{çÓ >öèˆrž?ïífWË¿?k¦xXº¿¡?b陨4@Ú?k¦xXº¿£?ïßn§*Ù¥?h‹Láº0!?pH¬j".C?h‹Láº0+?ïþÝW'n–?°­ü±'ç?"*†é–Ñ?°­ü±"-3FGL J2119.2-3313@'›ÙÀÑÀFê jšÀ9ëãïÿüÀ:ê ;ꊿè6+±<V%@ñ0¯J@ÐÀ¤ ^?îtXûLo£¿Ø	2åk»K¿ì1Vë…ZÙ¿Òàò¹pyAGNbcuPMN J2118-3316?﵎³/j§?WÀâECÏ?'œS4%V^?WÀâECÎ?ïòOà!n3?f¹x5‰?[`?½#™r?f¹x5Ž?ê($Rˆ¢£?°ûqè ô?Ç_nµÝup?°ûqè ô?ïø÷\N?Q9Z¯?L"§úÂ??Q9Z¯|3FGL J2121.0+1901@QPàÑnÀ5A/¨;ôÀ8iÎÜq…~À;FŸù/+g?îrIƒ#,ø@J»Þ'òá@DŸWž¢¿à‡àUÆ¿ã0ÅDÿàã'æ&]¿è¹;–
)AGNfsrqOX 131?ê33R¨"?ÃË£gW#?Ç32µ_®?ÃË£gW#?áYÙp†.Ý?Ðzr‡;?ÝLMó¢E?Ðzr‡;?çÂáÔÚ½?¶òÝæӈ-?Ð{ð<VJ†?¶òÝæӈ-?ágx8º1?»ÁsZ~_?Ýé1Ž‹ž?»ÁsZ~_3FGL J2123.6+0533@Lüa_–hÀ> KŸ:ÃJÀ9í.÷<À;®á?J˜«?ÐU5åGËy@H°Vï¦@`_ÂWÿ¿¸
PíПã¿åk\¨U&׿âGÁÌ#ë©¿â<I}³›4AGNfsrqOX 036?ïþJcÐü?3'ÈÞ.˜?+^yÂð9Ù?3'ÈÞ.~?ïã⪴ë?réìT7Ò?lUKüc?réìT7Ñ?ïr»
–Ô?†´V|ÔðR?ˆ£Q<šJÀ?†´V|ÔðU?ï"/Ó¹a?v äÉÂ\l?Šô˜§y?v äÉÂ\m3FGL J2124.7-3358@%ß# îøqÀF¹ÿÅGÀ7õˎß+À;MÀ‡D,€@ªaèÓ>@Käÿ¬ä?õƒ…UE¿¨¨ƒþc¿ÒPòÌ:֖¿ä¨‰{¿ï"å™ç+PSRPSRPSR J2124-3358?Q±OåùR?IkG	!jx?ï÷'?X
?IkG	!jx?ƒ¾è		%~?€$»NÙµ?ï±_ÛÛi?€$»NÙµ?…ƒ¶	=?†Ô²G
™?ï©óÝ'Û?†Ô²G
–?(êÍ4l•*?$ç:[>	?ïþqS,¹7?$ç:[>	3FGL J2126.5-4605@všßµÝÀFÒf€g™lÀ8Fo?Rü&À;….0Dk?ñÌs)˜U@nšúíœ@¯àÄ¿âúz§]sñ¿çžâ¶:††¿çê^¹ÚèÕ¿ëøSçïÏAGNFSRQPKS 2123-463?ïõ8ä±Oî?PR•Ê÷û$?UŽ6`$€?PR•Ê÷û3?ïózûU/0?d÷ š/Ï?Y
	U¡Ÿ?d÷ š/Ì?ï餇·Ä?" §ëeáR?Ÿ¢Ëo	?" §ëeáS?ïù•V8·?GœŒI§k?I«ö§#?GœŒI§P3FGL J2126.5-3926@ú'À9@"ÀGÅ 0!0À:^
ÒPšÀ;ç;¥È|?Ýv­©ÏzZ@
eWСm£@ŸÔà—"ì?ëíÏ¥³òû¿á
§ù®­'¿ß¡¶{%Ò¿ïÿuQCr#AGNbcuPMN J2126-3921?ï"[$Jüô?­µ[yw#?›´›v a?­µ[yw"?ëL"?ý•[?ÅçÁ×3"§?ÂÏw	ª—?ÅçÁ×3"§?é–ÀFæa?·?RÜÄm?Ëí¤þäf?·?RÜÄm?çÝ-"è"C?»9ËøŠ–?ÐE¤Ø.Ùz?»9ËøŠ–3FGL J2127.7+3612@T֟ŸØwüÀ%%ó_ÍTÀ9\M}À;DÈ6eÛ?㛽®CA@¼¿ºÀ…Â?þb±Èd¿Úè—-®¿áDâŒôçë¿Ô©fK
šr¿Þ"%öx†"AGNbllB2 2125+35?ïAõ	/?•#L¡™?—Á^ÜZ7?•#L¡™?î9|¥è+¼?µ©?<?¬h5¡}DI?µ©?<?î°J2<+	?˜þ
Dž
?¤û\Ü=O{?˜þ
Dž?íN¶´ibþ?š.{óS­?µŠJ\´è?š.{óS¬3FGL J2129.6-0427@Hu9ÿÖ•ÀBsÇä¡ÖÀ9G¢[	;À;"ËÚ^†?ôß»6¢S|@dëÑëþ@½' Pˆ¿Ø]:vQ¿â©'…UêÿçY¤4ŽcA¿ìŽËj!0ýPSRPSRPSR J2129-0429?¤,ÿZ?¥65gŒ?î½> ?¥65gŒ?âëùmh·?΍û_+¿?Ú(
%Ã."?΍û_+¿?¸<­­Æ?¨n•Stï?ìðjJG@?¨n•Stî?Îê¡L{ø¯?°ÓՓ?èEW¬áÕ?°ÓՓ3FGL J2130.8-2745@3ÿV_ˆ%ÔÀFéaÀxiÀ9àwŸsÎ.À;¾:bÒ]?ðÍB"xm@
£*ƒ6UÒ?û-_ÿÄñ·?ï:ÀÎÅS?íãqàÃr¿Ö‰í›	Â]¿áoxæñ'AGNbllRBS 1751?ïÙ¯ûVªn?w-éÞ?s(TªÈ˜?w-éހ?íÁs…'c?¸<¾N°º?±ôcÓoÄâ?¸<¾N°º?íPS/%‡ã?¤2UŒð®?µ}f†ÓÀã?¤2UŒð­?æ£Ã¶pIt?ÀÃÌRfí?Ò¸x"m?ÀÃÌRfí3FGL J2131.5-0915@Eòp_äl&ÀCÕQßƤ•À9^YûIÀ;…¸¿Þ¨?Ø´öp£ðÏ@߂ÃiKÉ@1ÿ¦™¿ÜVÝaÅlÜ¿ç€À¶F¬¿ÛOt2$¿ÆW†àÀ†AGNbllRBS 1752?ïü×jH™´?8Ôug2Î?9D­»2dü?8Ôug3	?ïí®€»È¸?lHIü¶ü<?bQD7Gn?lHIü¶ü??º%?‰Pº ?Œº'v˜¢?‰Pº ?ïɽ>Rÿl?q)`u4Ðø?{!`րIÐ?q)`u4Ðö3FGL J2131.8-2516@7‹yœÝòÀF½aßîèÀ:C(ǀÀ;×>â"Þo¿÷Æ<lí¿@´Ô©˜@ÿÿ&§¿à¤\—ÊP`¿Ú§Û%Õý¿â"Ò«Å&v¿Ü.ÛHP7AGNbllRBS 1755?ïü/ÕÆá:?CnÈÎÇÆ?>QÈö:†?CnÈÎÇÆ?ïò²¢Ù#?fé–¶"&?[šºMºt?fé–¶"$?ï@ýz7k$?'êhy©òZ?—àP¹›u?'êhy©òX?ïþµµu[Å?'žvp-Æ?$¤¨ªCª?'žvp-ÆN3FGL J2132.4-5420@u]8À>-ÀFqEÄÁfÀ9Gíf H
À;·¢šÊB¿ë¾É e@d¥‰çÊÕ@X`"?h¿åÊv''²¿é´ìӟÇ(¿á†1/D^¿ëˆÎé¿7AGNbcuPMN J2132-5420?ïÿaÃݚs?³È¿ôß?DŽL±£
?³È¿ô.?ïòSÓњÐ?fKI:´÷'?[XX\Ê]Ž?fKI:´÷•?ï͕éO×½?xO÷=71ä?y5X"*?xO÷=71æ?ïþëƒÜ(?!·`Ø?!GÂ6-Ô?!·`ן3FGL J2133.3+2533@Sy?ò^WÀ2ñ1Àll:À:IÑqw<À;¥É¤úì¿ìþgƒ¿4*@
Ÿ3«S*t@çU ›¿ìxÛ¢S¿×gb!sK¿Óþ;ĕ¾¿ãÞ
ùÇñ`AGNbcu87GB 213100.1+251534?ïü[ú{2{?<*ó'$¡?= ,&l "?<*ó'$Ü?ïÑö*ʇ?ƒ~‹óGÍ?w~ꚼà?ƒ~‹óGË?ï½×ú3?y¨Š¡¨?€º¿Šs??y¨Š¡¨?ïú6*—÷?FEÉÉüv?G'U£ˆ 0?FEÉÉüv3FGL J2133.8+6648@ZLhß½jY@&5Á'ì¯À8öüšòÀ;Fçž	jãÀ»zgODŒ@·5Œ©Ç@ŸMÀ¨&O¿çv\{è¿åŠÝì&PÄ¿ÅõJç¦9¿Þu&HÐ9¥AGNbcuNVSS J213349+664706?ïÿÚ@¡7á>ðâˆóã&>ò߯dÃà>ðâˆóã$é?ïå¯í8¼?uË`·"?jPÇCæM?uË`·"?ïèěð
°?s%ÓM2bÇ?g;dõO†?s%ÓM2bÅ?ïÿÿ4(¢>¬¿53°$n>™}úë´â6>¬¿53°€…3FGL J2134.1-0152@J3lÿݛQÀB>Ÿ¾vÉÀ9ÂzcÀ;‰Ê)"]È?êåúr¹9@_Ə@¨õ (š¿Ûk–/§¿åB¿©^ð¿á*èàÃh¿éžäq%©AGNbllPKS 2131-021?ïüHð+'8?;ª}Šïmr?=¸~£v>¶?;ª}Šïmd?ïë›Q;¼Œ?mõúÕTu"?dd®ÄCu­?mõúÕTu'?í¬æøºÐ?£€3×ZÞ?²˜È:){‹?£€3×ZÝ?ïàSÌH?`ÿ#žýò?o¬3·pü'?`ÿ#žýò'3FGL J2135.3-5008@u·©³únÀG1Kÿ²Ó'À9&*·c®üÀ;ti;'§?å¦Qs˜±›@/Á™gð@Â7r@º¿â]Pì4Nſ磷쯯õ¿æ
fyG¿î97²ÚïaAGNfsrqPMN J2135-5006?dPeˆ?ŽNßɘxÌ?‹fëæž?ŽNßɘxÎ?ï@9'Ö?Ÿªý{ÏD?—üüØÍÅ?Ÿªý{ÏC?íñ`·j=$?£°ï´´1G?°túD®Û?£°ï´´1G?êØɆ?©j¥Æ͈?ÇôŸçÄÙå?©j¥Æ͇3FGL J2139.4-4235@vdڀIf{ÀH)οìºÀ8àÇU"‡À:ýÂÅ+?öùŠ¨ex@ðÀêÁTt?þ.` ©®:¿ÚÚ$¿à‰ñ]]%¿âª-qI¼¿å¹·©AGNbllMH 2136-428?ïûÐEK"ä?Bªdl`?@¾êÑ°i?Bªdl`?ïíÝ#òª?m
5EXG?b"Ü
Uäì?m
5EXG?îä›'7	û?–ŸT'ôï?¡¶MŒ`@?–ŸT'ôï?ïŠiQ¥'ï?†ù¡(ø%Q?e«–›"?†ù¡(ø%Q3FGL J2140.0+4715@W(üà%o%À-J?¿2°À8~&vŒNWÀ;9ÕÓ܋‡@ÆèVÁ@
b)Üó5—?÷òˆæüy?ƒMc¤ÙØh¿ßæ碈x¿éÀ9ÖæV6¿ïÿߓpW"PSRPSRLAT PSR J2139+4716?b¼OYÅ&?hò
_]qª?ïíC°¦ì;?hò
_]qª?C-ç©ê?Y]žrçÁ?ïû4†À?Y]žrçÂ?¡%ãâAÜ ?›§húIùƒ?îí¡ÁÛâ>?›§húIù}?6 ]Ð̊A?,'e
±þŸ?ïý+ôEæo?,'e
±þŸ3FGL J2141.6-6412@t‰¢ß"xîÀE!'	±À8úÙ*© öÀ;¦þÍÐØË?ñ€=û8E@"ž­Õ'@ö?[4¯¿âuöÉk¿ço7HŸ3À¿ç>‹Q¾tÖ¿ïûdÒÁAGNbcuPMN J2141-6411?ïø‹ò"r…?N]'õ3î–?MÐ7v5é´?N]'õ3î²?ï~Áñ?f»H…ŽÀ?`pX>¡?f»H…Ž¾?ï7LëV?"yՐ16?™'•<ù?"yՐ16?ïד>7m?jcµ6õ}È?t6`äI8ä?jcµ6õ}É3FGL J2141.7-3734@|XüŸ£ÀH…ÅŸ±áÀ9º;Ú¡¡¦À;ÂÊ榓¿Ó$šß>êL@ÿ<ú\R@»e€À¿á·b¾w¿í$FŐk¿Øm<7­…#¿çƒÔ¤˜·XAGNfsrqPKS 2138-377?ïÿûæ_ç>ÃÜ`'Åõ>Ãìf€ac7>ÃÜ`'Û¢?ïòsÉrÍ?f՟é,œƒ?[meþf?f՟é,œƒ?ïéqO#™õ?mÛr8{a?fŽ°Üfü?mÛr8{a?ïý*–Ôu`?0åß´Ðñ?6«I\U?0åß´Ñ3FGL J2142.2-2546@7œà`'ˆÀGòˆÀ-'À:õÊdÀ;ÎþV²"<?âþŒ2'ð_@ªÅ[>j@ىÆã¿àÙ24Z¦¿áø'ÕE¿â@ª½áÕü¿ïþ½FSþAGNbcuPMN J2142-2551?ï ¦Ö·¼y?Ã"E_å?‡ÖJRá®?Ã"E_å?ïuJ¸i<?—P­±'?'V¨òØ}1?—P­±'?ìÜï³?¨ìÓ%%Ü°?¿g'gÜ?¨ìÓ%%Ü°?ì«f_¿ú?£gdEƒSò?º¤Í*5?£gdEƒSò3FGL J2143.1-3928@´j¿f‡ÉÀH¡à f§ÕÀ9å)*›´ýÀ;¼÷üü??Ð9å©èqC@¾9Èxª6@•p@"Õg¿ãù/±¾¿ãSßÁy»¿ã_Ø{4\\¿Ê´ûÀ¾2AGNbllPMN J2143-3929?ïÿ%Á?Owà™2?B+)‡á?Owà™
?ïó—íuF®?b{«¹
þÔ?XÐ%r¤‡?b{«¹
þÔ?ï½îÁŁ?ƒbœ¯ûE)?€"OŽ¿_—?ƒbœ¯ûE+?ïÙNöëRÖ?i§c×bš?sX"ŠV•Â?i§c×b—3FGL J2143.5+1744@R~_ìÏ¢À:›?Œ
À7ykˆWÀ;™À0X?õ'–‹SH@TI,į@Ò"¡!¿ã·+À^f¿çš+FC ¿è·¾-‰¿èќüê:¶AGNfsrqOX 169?ïødE/jV?P»áY=Hö?NnëBV¦b?P»áY=Hð?ïÜCÞ÷"?yÓço©"ø?qÞÀnk?yÓço©"ø?îï8¨~¸?—$"¸Ô?¡uxt'?—$"¸Õ?ﶔûyýž?~9ß_³¶§?'ZÁ!€˜–?~9ß_³¶©3FGL J2144.2+3132@T¥µà!=gÀ0Kæÿ}úÀ9©°â‹zóÀ;¡­SŠÁ?³ð˜-›µ!@A]Û}i¸@å¾@Q¿æT-';¿Z¿èL®ITè¿àvÒ&î_¿ØýNʾUAGNbcuMG3 J214415+3132?ïúóÎìý?F&W\	?D0ÄOÄ?F&W\?�,Ç	?Š_>Sb"™?€?´Î=Á?Š_>Sb"˜?ïµÎ¿O"?-ØæՀ?'ŒP?,{?-ØæÕ}?ï¼¹`‹?r—ð&W?€ùü§Üõ?r—ð&U3FGL J2144.9-3356@&ó7z>ŠÀHÍ«ÿÍ«À8÷¨§b°À;¸£J"?ça{aŽÿü@f2R7°@\–Þ²}¿Ú‹¨-¡¿åŒv¢¾¿å•GÄø¿è}
xAGNfsrqPMN J2145-3357?ïýѱócó?0«án?1rpdàsy?0«ámæ?ïó¡Ðt¶L?b†«¼þ6–?X¼_"g©?b†«¼þ6–?î°@ù*É?š$ë]ƒ$[?¤ûðn}Sc?š$ë]ƒ$Y?ïù@Ø?Cjz}õ?K‰û'ü¢²?Cjz}ð3FGL J2145.7+0717@OÄ"}À@µt@C¼îÀ9¢ÓßÅpÀ;‹N[­¥ÀÀ'(–ÍŒ@—f´=@@m`€žK¿êö¼»:[Ï¿æõ;4A¿å}©gå9¿Ì#â.‰AGNbllMS 2143.4+0704?ïü»ˆr¿ó?;ýåàVhœ?:#¼jeÆ?;ýåàVhÂ?ïïåÒ\Ÿ?m¼ì+÷C?`ó-£a?m¼ì+÷B?ïiuÿvo?‹ôâÓÜ?'Ñ@12#?‹ôâÓÜ
ù?ïÿõ^ý>ÝRØ\$r>ÕïBÞi\>ÝRØ\$£3FGL J2146.6-1344@DT—b%ÀF|ŸïôðÀ9sñidHÀ;t•?ñþIQW¶u@þ¹+ZKÑ?ú}ÿµ,r?ï°'D"?ߦW{¯\¿ØÒùmzèæ¿ÒýGbƒò'AGNbllNVSS J214637-134359?ï›ó',ýï?‹¬½bÒ§?‰tÀ"?‹¬½bÒ§?ï³ÚaCñä?‹Ù¨ÊÖ¯?ƒ	g¯‡?‹Ù¨ÊÖ®?ëÔA—^#?¬\ÁKj?À®ù¢‡÷o?¬\ÁKj?ê;$qÊ?·ž:nM"?ÇÃn8׺?·ž:nM"3FGL J2146.7-1527@C:\?›÷BÀFØäÀ™,À9åVI¸±À;µ5õ…R»?×¹¬%¯´[@Éª@«À#Ç¿ßíÔߟ¿è¾Zâ,c¿êaJ"wbQ¿ÌO¿iüŒÈAGNfsrqPKS 2143-156?ïüôS
S<?Tw#ö Ñ?8]g•fp?Tw#ö Ñ?ïòtðþ?fª»z†Mã?[Óä»?fª»z†MÞ?ïCNÃsG?'F¢°Åèz?—–''—4?'F¢°Åèy?ïй(Ő?r+3ò`ޔ?w£k7ü?r+3ò`ޚ3FGL J2147.2+0929@PsìZþÀ@#%¿­)™À8·	)7À;?ä^¹É»?ö‡¢äß@±·Å(¾@µƒ.ž#¿áh¯¶ˆà¿è‹A".¯¿èn~K=Ë¿é}ÆTb­ÊAGNFSRQPKS 2144+092?ïù¸{J¼?Füèì£!?IÕ
þ|?Füèì£?ï笆\‡‡?t~…»$ù?hSy£xx…?t~…»$ò?îÛcÄó'?–œ³n~B:?¢IðÆæö?–œ³n~B9?ïóÚ¡KUg?TV©—;Ü	?XJ½iU/!?TV©—;Ü	3FGL J2147.3-7536@s¼®_ú;›ÀBD-ó»NÀ7[ðEwÙUÀ;/†è¼í\?ø˜‡Ô3s@Û6"Q@rÑÊãh›¿ã†ž%€©D¿æ销w
¿èÝz!·¾¿é@«}‹ŠÒAGNFSRQPKS 2142-75?ïøæe7YV?I‰×.÷	8?Lfk"š ü?I‰×.÷	%?ïg¤?m§ÿÕ?aFræ˜\Ÿ?m§ÿÕ?ïLéЈf?"ß"ìLÓ?¶bÅîó7?"ß"ìLÕ?ïÿÅwŠü?ŸÛ¯*à>ýD:ò'aP?ŸÛ¯*˜3FGL J2149.6+1915@Rœz?̞ªÀ:
Û L¦¢À9VÆu'ÊÀ;sCWm¥?c©te%_@Sz'î.Ç@Œ' ;¿å
ª
7ԋ¿çE¹*-¦¿ç›@'{Ï¿ïÿîpǤ€AGNbcuTXS 2147+191?ïÿ~Íêi?-1Rq¬?<†B³ˆ?-1Rq¬L?ïÛµ-t
q?}ֈqãIÀ?r%iEùH?}ֈqãI¿?ï™u!ñ?‡SxìT°?‰¢·œ8ë?‡SxìT°?ïç]‹Üå?a"$våö?hù¢t#A?a"$våý3FGL J2149.7+0323@NFâ?û˜'ÀBQ,_Ú[+À9˜ÛÈRéÀ;©¼®q—ó¿Ö s8ז@ÖJHùn@4ƒPþ¿ä{Ÿá1]Æ¿Þsñƒ)Y"¿álš¨7l(¿è|/՟sAGNbllPKS B2147+031?ïùYä0ý?MÃùºâù?J˜o<·¹?MÃùºâ?ïã »LÔ?w™1^¿u,?l߀D³->?w™1^¿u.?ï=·KJ?"E8l¼Â~?˜IŸ6–¸?"E8l¼Â~?ïر³}?k'X€ËÏ?s§7ý&AÛ?k'X€ËÌ3FGL J2150.2-1411@DMþ_ìÏ¢ÀFú?Ï"èÀ9ÉΠ£¢À;‡ìZ0Íþ¿ó9‰®¿ñr@Â}'Þ[?ýB"!=ƒ¿ãYß­5i¿âÂ:Ƌ¦M¿ÌZMN¿ð¿â‹t™É®úAGNbllTXS 2147-144?ïÿ­À…È×?ëA韵w?ÞÊaó?ëA韴ƒ?ïô‡&ºJ?bË´|qõ7?Vñ²‹ám?bË´|qõ<?ïà4kÒC>?o›<ƒö?o˔-¼Â'?o›<ƒö?ïÿhâRdç?
9@~?ãµ³c,-?
9@ö3FGL J2151.6-2744@5PÆ3¡îÀI*èà(Ê$À:'e"'ÒÀ;Ë5™?Ç?Û/ú?\ó\@/‡­@Z€a¿˜"³ƒ´o¿êÂ#ë0¿é­"b€~¿äÔ%¥<KFAGNfsrqPMN J2151-2742?ïí:Qýÿí?mŠ"ö'þ?bÅ®×?mŠ"ö(?ïáˆÂûð?w²-Ç¿ø?nw=â?w²-Ç¿ú?í'ÔuôŸB?¢V¸I¨<?³i\P[í?¢V¸I¨<?íØq½Ä°? c"~
Øí?±<rۂ†? c"~
Øí3FGL J2151.8-3025@1!Ef­ÀI`Æ báwÀ8>ŸªÀ;cá6]E?üó¥&@"¬Âc¿@	Eç#»¿çŽ:¼z«S¿íÒ_³Ä¾¿ï+¢^Ô¿ïç®ÀGXYAGNfsrqPKS 2149-306?ïø™8•L	?Zí^þLç?M›ªÏÚ¼?Zí^þLã?ïíòô(:}?u‡ætí£×?b
×Ń3?u‡ætí£Û?ì†ûÁìÝZ?¬MªD[èÚ?»È!ð™4?¬MªD[èÚ?0ªË?ŽY‡ýõßü?sÕzÍ©?ŽY‡ýõßü3FGL J2152.4+1735@RidÜY2À;±< BÀ:"曪ëÑÀ;Ï"‰G<?Óuö
°9;@LxiOò@i3ˆf¿ìn'yÂc½¿Ò¨-}‰¿×'e/뼿çÎM¸<yAGNbllS3 2150+17?ïïÝúµ,?coÖ@Æhq?`"ôJÓ×?coÖ@Æht?íøJÂË[?¹2…ÇV?°=©ïY¥5?¹2…ÇV?ïg d`?éK{Ð;ð?"ëóÓÜ?éK{Ð;ç?ëm'è4?°¯6q¦?ÂIô_Î1?°¯6q¦3FGL J2152.9-0045@Lw©Àª€ÀCÞÆ_ËA²À:I´+'À;ªÕ¥¹cÀdfÇ_Oœ@=½O?ÿ)"_è¿ê¿«4²ËU¿¯anAž}¿èòÖ¹¾0?Ñ]²eöÝuAGNbllRBS 1792?ïô6mìG{?WºŒjÎËË?W"$'q	/?WºŒjÎËÇ?ïò‡"á1?eN^çã¿g?Zñ»Ì=œ"?eN^çã¿l?îê1L7Ì?"Ò©Ë»šÎ?¡\ë<Ž"Q?"Ò©Ë»šÐ?ïÿçJ ‹a>ó¨y¥VV>èµ_tŸ
›>ó¨y¥WÝ3FGL J2154.0-1137@F>T2TçÀFÔÓßæ…À9:̎¹kÇÀ;ª¬ê¯5ã?î"Uk±Ô@}Ísí@é(€&ÖÙ¿â@4XLGV¿èO'²v¿çƒÉü¿ïÿíÊ"EAGNfsrqPMN J2153-1136?ïÿ[Ø"?
¯©…Á"?T"û½	b?
¯©…Áñ?ïÕWïpÌë?'Œ«¢WT?uTG™Š?'Œ«¢WS?ïT@U…HÀ?Ž	í)(Lä?•wõOVè*?Ž	í)(Lã?îNÎ`Eš<?›¥ò©Û ü?«û¦\3?›¥ò©Û û3FGL J2156.0+1818@Rº6ŸÏ=ÀÀ;Ê	 '²À9ôW(ÛÁÀ;š}=B€®?Ç`d×ù"C@¸]?÷î?þ `"=µ?ïüà*D«¿ãÿl(¿‰¿ÓäŒ&iv;¿ãÓ7m©"AGNbcuRX J2156.0+1818?ïÿ!Ž3Br?!dZÀؤ?Î9—±Ÿ3?!dZÀص?ïÚ]½¤;e?{f÷üwÑ?rÑ!-âM[?{f÷üwÑ?ïÂ,G¾V|?}Úøî
Üù?~éÜ ÔÂR?}Úøî
Ý?ïÍ\‰dÀ?nQÖøH•?yQ»p͟ˆ?nQÖøH3FGL J2156.9-0855@H.­@?‹0ÀF HtäÀ:t䝣êUÀ;Æ£iüóÜ?ÁÜ#¾r@M¯gQî?þm'Ԇª?ïñ½øÒì?ë£`Æ>F¿è'ßSª¿°¶¤cC"AGNbllFIRST J215650.3-085535?ïÜhM>Y´?ˆ"Øx'×?qËÙ`Ó&¼?ˆ"Øx'×?ï윰Ø=¡?uÅ©1‰Í?ccO'Â^Ö?uÅ©1‰Í?íkÆÇè?¨å¯Þa?´¡Ï1À¿X?¨å¯Þa?ïŒ(`–m€?'Û:fô•?ŒõçÚd -?'Û:fô"3FGL J2157.5+3126@U0m_êKcÀ2=²?'ÌÎÀ7ž1œZ>:À:ôŸÅ,Å[?ýºOq­A@¬:ŸŽ%G@¢ø{§@¿Ý9: Íâ¿ã–δ¿ û¿æ_8`ÞUû¿ê¡¯`¼iŽAGNfsrqB2 2155+31?ï*3ö7d^?˜
‰µ·ã?š¹9t8?˜
‰µ·â?ïÐÜ÷Ò ª?"mlªÉ>…?w'"¯«`?"mlªÉ>'?ç—Õ%f"?³"c|^v5?ÐÐUµ2×ð?³"c|^v5?ïö'­+Öe?RZÕNC	8?RÚ¥¨S6Î?RZÕNC	-3FGL J2158.0-1501@DOs€*\ËÀH ö½À9+äŠYÀ;"C/Ш¿óòúX¡,@^‰x9M@'Õ`EK¿ãyGë=|¿ãàã»âÕß¿åu(ÐGšb¿Ûª{4åÍAGNfsrqPKS 2155-152?ïþéüÒÔþ?&iõMÄ{?!`2Ò°%P?&iõMIJ?ïóâ¡æ?dÍúyÞÃ?X:¼3ÓÜè?dÍúyÞÄ?ïi¼šf¦Ã?ŒŠõ3îT?'Èl³+'š?ŒŠõ3îT?ïÿĎ½<À?NНÆÄm>ý¸¡aŸæ»?NНÆÃô3FGL J2158.8-3013@1º¾`"‡ÀJã?ÕØåÀ60Õñ8¼àÀ9Ïù‰Ä:?ðÚº1¦k@µŽM5<ù?ûCÁñQ'm¿Ò
¡ÞPr¿Ý[4Z5窿ٯ ›¾7¿Ú@µwp¤ÙAGNbllPKS 2155-304?ïé"eªÑ	?{&_Q˜õ?f{šU.öÞ?{&_Q˜ù?ïô¾õ昞?d÷:!2"?V'2ÎÅ°?d÷:!2‡?ì-o.è¡O?¬æTçcp?¾"†ˆºõŠ?¬æTçcq?ïÿFÒË?ß4‹L?%¦»?ß4‹L½3FGL J2159.2-2841@4<ú?̞ªÀJ¼ .ßÀ:¨y0nÀ;´ÆžµbM¿áäò
¦f@Øe-VOm?ÿSßûþ"¿ê³A¥*¶&¿Ü1''©Ô¿Ò	nÕ1˜¿åG‰óD—AGNbcuNVSS J215910-284115?ïÿ~Ì?™\bùvâ?0=Mæ˜?™\bùvH?ïð™ÓÅ&?jUÕ †‰"?^ÌXu˳G?jUÕ †‰ˆ?ïÕv"&¯?r+NIq?uD½øì¨Æ?r+NIp?ïùWõ*?F#vÍR]í?K³' +UÑ?F#vÍR]Á3FGL J2159.8+1025@QFàà¨.À@ú0ߛÜjÀ:þñ´
À;µu	—Xw¿ÓK!ÄÿW@ùô+¶g0@% Jù#¿êS?V›ÜÚ¿éλžônʿȑDá[z$¿ïï{¹ðã>AGNbllTXS 2157+102?ïû]Ô?S0TjÕ9?B‹À¯ÿ¤y?S0TjÕ:?ïÔó~yˆ?}GüU/ˆù?u†ÀÃ<?}GüU/ˆ÷?îÅc"$8?š{7p?£¯ùƽ¼"?š{7p ?ïÖ¨VŽ ?u§=˜x?t«Ô¸ö¯¶?u§=˜x~3FGL J2200.2+2139@S'tÀ0ÝÀ:6_7üÀ:°àÝûÉÀ;Ý`ÖÚlÉÀ.Ð ¿=B@ŽdŸfã?ÿ£k_I'™¿íx[â»ã¿Ç	$6@-í¿Ø]Ÿe`'¿ÒQh3VTÝAGNbllTXS 2157+213?ïþ՜®)?0«@ esÁ?/¦5e"?0«@ esÖ?ïç%mêøÙ?p‹ôX‰)P?hڒ'±?p‹ôX‰)R?ï©#9ŒÇ¥?€dJ¹2ë?…·1œÎ?€dJ¹2ð?ïÿÞ]ØÓÇ>þ°þ4¸þ>ðÑ–÷¥>þ°þ4¶¡3FGL J2200.9-2412@;}"V!uÀIÓÝà‡kÀ:H%"ü|À;â½ F?¥½9…'‰Á@e›»2@¡³_¾V'¿éƒëûnÔR¿ëuÄÓ·«0¿¦õ§•
vi¿ã)åz©Ð…AGNbcuNVSS J220036-241428?ïÿ͚)ŸÁ>ü*©±xÊ>ù2ë0ß©>ü*©±xÈ?ïóŠ^i–?e¡ø‰ï?XëC-Ö?e¡ø‰é?ïÍ9Ôs›?w0¯RÎEç?yc~•Æ2Æ?w0¯RÎEä?ïòS#¤ø?T€¶ +?[ÏY¸¶÷?T€¶ +3FGL J2201.7+5047@Xi"d¯À^ƒ¿èÉÀ8).‰À;5/»¯n?îkÀÀSJ@r'2Ÿºp@¶Óàg^^¿ä$`gÒTÕ¿ç6ÃÝ©­¨¿è®n4]w!¿ï3Š!oAGNfsrqNRAO 676?ïªùkÎ?ƒæ¥D8]?…A¥?¾L•?ƒæ¥D8\?ï
Ÿ0Tæ?²kGh®Ø-?ž½ìõcY?²kGh®Ø,?íõã7\? z.å¾U8?°PçvE…? z.å¾U9?ïÿù(j#–>ÒÝ?Dۗõ>Ë^Wq¥üã>ÒÝ?Dە93FGL J2202.4-8339@s?÷LÀ?¼±v/À8}¨'j¨ëÀ;³¦‹¤?ú>ÿ'ö×@ºæ´Õ_C@"?(ßÈ'¿áðÆËÅ«¿åÁªRàˆÓ¿è¤ÃðÉðé¿ïW¶ð9üAGNfsrqPKS 2155-83?ïˆ9Q.?ë?‰'ô1¬À?ñ«´p1?‰'ô1¬Á?ïäì@?su«Ü°¾ß?k¿áþøì?su«Ü°¾ã?íJ¯sá&'?£gJióñ"?µª"`öËs?£gJióñ"?ïŒ>É_˜?ŠÉ¿&yR?Œðͨ@?ŠÉ¿&yR‹3FGL J2202.7+4217@W&@_×,À$á'ÿùJÀ6t _ñØÀ:…nÉw-?õôò°·@0áhv@ã±jƝ¿á€…15_¼¿ä©§…âÏæ¿ãÚÓíõ³Ã¿å±ë`œßAGNBLLBL Lacertae?ïë^ŒÞßÈ?hBékèzª?d¡s! 6á?hBékèz¨?ᅫÜ¥?ôzÔÊR—?€Hù–¸•?ôzÔÊR•?îpi"´úš?Ÿ¼ÞVø]f?¨ùf´°VW?Ÿ¼ÞVø]e?ïÿèIÔÑæ>ò[éžÌAÀ>ç¶+.ÈC>ò[éžÌ@V3FGL J2203.4+1725@Rëà
ò1À=£GàiaÃÀ7»Šˆ"ž`À;Šrµ)B?ñååóö@ڜ#·•-@QâZþ~K¿ßð0$ò¿ãðk"LD@¿æ!ÓÉã…ÿãSù¼;|zAGNfsrqPKS 2201+171?ïüL·Kǔ?>gdä?=šE¡Ãa0?>gdä?ïê°UFY"?pˆ€S,?eOª¹¦Ý«?pˆ€S)?î}Õ"3j?š×ZÞnÙ?¨"¯Æ¼Éo?š×ZÞnÚ?ïûŒ-ÏZ¾?BhY?AÏH•…?BhYŒ3FGL J2203.7+3143@U¸¿ÏŽHÀ2ރàÊ°"À9 Qðœ5À;Pf͔ÀŸPõ-¿@'=Ì¿5à@†‡_ZX'¿çšøO:c¿éWÝ÷cñŽ¿ïÿÛ¾"_T?ÚW·€¤AGNfsrq4C +31.63?ïþ2»á°?1/í4IâÛ?.\ÔAå§?1/í4IâÙ?ïݾÞ•ñ?}d¢6çö?q ðµ$?}d¢6çù?ï
WԖÜ?ˆ‡¶-ºäq?Um$O?ˆ‡¶-ºäp?ïÿþÎñå>°]']àôÂ>£á¯¯.>°]']àÉ3FGL J2204.4+0439@P.lŸÐë?ÀCSçÖyõÀ9îévQÀ;Ãr°÷"0¿Âîªzüö@^Óª¬±@þ=ß^ŸÉ?Ùlé™BS¿ÚB»ú "R¿ëM豍^Ö?²uµ"(üAGNbll4C +04.77?ïØ£ÌYå?w%'ÿDž?s®óS
à?w%'ÿD¡?ïñ³28}Ú?cåù½´ó?\™›N€?cåù½´ô?í¬*äÙo?¦™Î)Ÿ(?²ž¯ðÙ4‹?¦™Î)Ÿ)?ïó	3D?X¼Ï;0ÉN?YíәáyJ?X¼Ï;0ÉS3FGL J2206.9-0031@Mú¼ßï¿@ÀE6ö`D
vÀ9¢T™µHLÀ;ªf̽³T?ÐXá"-nÎ@Ûhêz1Ê@üâo\¿×âK€K¿âæ‹Ôx×q¿ãï/Z¶"â¿è~ %ò$mAGNbllPMN J2206-0031?ïÞ{™Rÿ¯?xˆô'åÄ?pÂ3V€(–?xˆô'åÄ?ïØ(å
\¨?|
b°ð?sëzÑ«Ž?|
b°ð?íïD]¢6?£ø-öh?°…ÝïžC?£ø-öh?îø$°ùH/?Ž'Óã:? }´ðk|þ?Ž'Óã:3FGL J2207.8-5345@u>…ߨq¤ÀHøm¾iÀ9ôÛö5À;̪â—9m¿÷?´öÂ?@\Ý%µ@ªå_ë¢ü¿ç~"ƒ
¿åCîÛ{¢t¿éjÄzÔç`úû©ëAGNfsrqPKS 2204-54?ïÿ‹Í'ƒa?*¶PÑg?
›Ÿ'ת?*¶Pћ?ïò¥ÆÙº×?fÆRLzBX?Z´rLŠSv?fÆRLzB`?ïº>å¸h¶?~\«C–›?pF'åÒT?~\«C–¬?ïÿï0@>碉'ÝÆ>àÏú忨¶>碉'ÝÀÎ3FGL J2212.0+2355@TŽH¿÷Ò4À:©?ÿÊPÀ9}K…9À;†ûß	?ÕKêßâ@,þ¯çÝ@²Ô (>Ž¿àÓý鮿☐MH:à¿ã«Àsß1¿ãr`†Â@FAGNfsrqPKS 2209+236?ïå½ÑÆë?p>Yäí?jB.ô9:?p>Yäí?ïÅÕóü?•^À=ÿ@?‹ÎŠƒøg?•^À=ÿ@?î:Àþ[…? mÓ®Fª‡?¬SðO÷¦? mÓ®Fª‡?î]PË>â?—
vÉÃõU?ª*þ³Lã?—
vÉÃõT3FGL J2212.3-7039@sôî²ÑÀD‡"€,á
À:${À;´»¶úÓp?ìû–dìúÑ@9`؇ëò@}\¬~¿ç£ÿ¦5UÅ¿è^VÚN·ë¿ìJ¦b2'½¿ÙaÿrAGNbcuPMN J2211-7039?ï¿£&rو?"‡Ë
5@Š?€6cIÉ?"‡Ë
5@‹?îPjŠ`Q}?¾ûÆìíe?ªùWYúè7?¾ûÆìíe?ìb3y_¤K?¦G¿ÓPRñ?¼îd5Ý ?¦G¿ÓPRò?ལ·›?Çïáª\ۇ?ބ¸'ýË?Çïáª\ۇ3FGL J2212.6+2801@UK2-LiÀ6û.Àë­À9ðÑ@±¡À;Qøñ?ÞwՋڋŸ@
z£?	Ö?ü¥ôÞä§_?îñÇ53=š¿Û⦖ŠÏ¿Ïáì"b½¿Òې
m•žAGNbcuMG3 J221240+2759?ïÅ-¡·%z?ƒëcOG3?}i/$mC?ƒëcOG4?ïÏØrÎõR?¢ZxÐ×N?xƘ…W§?¢ZxÐ×O?ïRÉ0=?'éöÞÊ?Õ¦Ùø]}?'éöÞÄ?ï)ÜêøÖä?Ò¸èú‰?šÄb å#L?Ò¸èú‰3FGL J2213.1-2532@:UC_Ñ ïÀKQìàh‹À9™TpšÀ;Ñ&çËUÔ?¼ŸáA+¢@íÓW«c@`e@ ¬s¿ãŠn'!¿åÌ3[t¿æ¬K¹xz¿ïÿõ•æ(5AGNfsrqPKS 2210-25?ïýº§šáŽ?A¿/Éúh?2*Ã(óÙ?A¿/Éúe?ï¶Ð_zgI?'¬
Pïù?'Kè!f-Ô?'¬
Pï÷?ïëëXšZ?–ð#%)~?Ÿ'"ì´Ž?–ð#%)?îß)û-?"ÊT=°9?¢
npM/Ã?"ÊT=°93FGL J2213.6-4755@uÀAà?pXÀJ"õƒ¥À:Ú'ˆ-aÀ;òABÀnð?dz¼G:ôj@ÇÉÅÜB·?þ;þÝÁ¿èeêG(ó¿c>"0hê¿äxiRÿ×;¿Å1݌|iAGNbcuSUMSS J221330-475426?ïÙN€ø?'äš…MíŠ?sXõ¿÷û?'äš…Mí‰?ïçdZÒ?~ÙD&׎ÿ?h›¥ó-þí?~ÙD&׏?R‡?"à²èÕ"?‰õ¯?"à²èÕ•?ï9U@á´Å?ìXþlÕû?˜ÕWãÉg}?ìXþlÕú3FGL J2214.6+3000@U¶¦ßÓ9ÎÀ5ª¢_:øúÀ8"kp'b"À;k/¬•õ @1Tc¯}@¦ÃMÈ
?ûÑE'ñ6¿œ³š~V·¿Û˜Û¥úó¿äºˆ‰&¿îwe_*\öPSRPSRPSR J2214+3000?P¾œ°‡"o?N½Šn›´u?ï÷ ±§¼o?N½Šn›´u?n"ZÂ3ß?u0•ú?ïák¥=Ìë?u0•ú?k±ó`V´?tšd*e?ïÁ(œ?S?tšd*e?Kó˜¯Í'?EÒÂ1¤~?ïùÔÀ?EÒÂ1¤}3FGL J2215.6+5134@X÷ÏÀ1³×À¹vÁçAÀ9žý†¨üÀ;WÊÆb?þ¥y+û¶@)"×ëŽÚ?üÕJœ?Ưåi'I¿Ûön+¸ý¿ä\z&.4h¿îÜ)µþLPSRPSRPSR J2215+5135?MŒX¡®?C"ó+‰	?ïøœú¸©Ö?C"ó+‰	?aŠô­ò°?oµPëâ?ïîîuR
?oµPëá?€×qÖ1ÿ·?q~>bhùh?ï¼¢8§8?q~>bhùw?˜•<îÔZ?…#6Ö±Á?ï;V‰_^?…#6Ö±Á3FGL J2217.0+2421@Tâ5`4>À:u§€)ÚÀ9;ٕ2+ÌÀ;‹õ'¾´?ä'ú¾z@'/ó7Ŕ@¸Š`¿Z¿áœ坠‡¿äÔ]eòßA¿ãªª=€¿¿àãšæîAGNbllB2 2214+24B?îaÉÛcqÏ?µ<«y"?©ãbIÈã#?µ<«y"?å<¬š`†ö?Ò°g¤n±?Ն¦Ë>ò?Ò°g¤n±?ëÅHÆý>Í?® bÏj?ÀêÜäÉ?® bÏk?ÛY€~q?¼ß~˶ä?âyÓ?ÀòÇ?¼ß~˶ä3FGL J2219.2+1806@SÜÝ?á—_À? íàBËWÀ9ö-Å5(×À;Ålґ2¿åŸLv{1z@Pš¢-@	qŸŒ¨¿áöͅô ¿è^ß®ü­:¿æˆ#Ó¢\"¿å¶"ÞAGNfsrqMG1 J221916+1806?ïþà8&—?!¸]›i÷w?!ÿ|}–?!¸]›i÷¾?ïèú<šÔ?r+[â~â=?g~Ãe-k?r+[â~â>?ïɖ ´˜Í?w¥ÔKrÃ?{4¯¥³™M?w¥ÔKrÉ?ïøAåŽÓÚ?Ecg?NøiÄ°›?Ecy3FGL J2220.3+2812@U°p@üÀ7ۚ?±Æ·À:†Tò ›ìÀ;Ëö³P$¿ê!È!õѱ@
SÙñÎd?ýU'Á(¿éð…ӿ݆³Äí°¿ÕjäJúm¿Ë²¹¹­AGNbcuRX J2220.4+2814?ïþZ[ÀQw?-eS^˜…ð?*ZCúè–
?-eS^˜†5?ïä7®&&¾?uÙžÒä®?kÈQÙÙBÜ?uÙžÒä°?ïÀT`Rzô?|QZšG°?ÕÏÖ†3?|QZšG°?ïý´¶¡;K?0¼¯ú+ùë?2ZJö%©Á?0¼¯ú+ùõ3FGL J2221.6-5225@uE¸Ÿƒ¾fÀJ2ûÿÀ? À9`^SrmÜÀ;Ó~—µ"¿ü˜V¶E ñ@+óSIS0?þÒ^ß´[¿à+hjìÅ¿àŸÜo4É¿¿Ú«`êG¿ÜšÖœžAGNbllPMN J2221-5224?ïúкð±—?A–DH»äO?D½=9¥?A–DH»äF?ïó3ëÕ÷?eBÐdÊþt?Y˜(Tå·?eBÐdÊþt?ïWRS§á?‹–¤ä?•µ‹Ý«?‹–¤ä ?ïÿTâÇü?RjIŠâ?c¿§¢?RjI‹Ô3FGL J2222.3-3500@#Lßàû®ÀL¨ñß«Ì¢À:ƒ¸:lãÀ<-*ÛuÝ¿ê‡Z'÷@Þ¬FD‡ï@ùã_`bÁ¿ãU¬žcË¿ßÕÖқT¿èÜÆè1W;¿ÖDf'§ûAGNfsrqPKS 2220-351?ïö8Là)š?`å#N÷ý?Sf?¬ËH?`å#N÷ü?ïõ@¾£Ù?`W°qâWÚ?U~'¸LùC?`W°qâWÞ?îìú8G?¡¼øü㬌?¨Á0\{œ?¡¼øü㬋?ïÿ»
Öi>ÿqaNéö?<Še¼U#>ÿqaNí3FGL J2224.6-1122@I$­€k`ÀJì@/šøÀ9öÌP¦
ÁÀ;¾ðù²¿ÿ9H*¼@
±Q؏Ε@'ªo÷µ¿æ‰¡Ñv¿è³ifƒw¿Ò0ыšÊ¾¿ïùÓKþ'AGNbllPKS 2221-116?ïñ>i:–?p³R'¸Ö?]ƒá-ŠÔr?p³R'¸Ö?ïìBcÒm€?vÅ$±ë»?c½œ-'€¡?vÅ$±ëº?8fnã?šQ¸w®?¦¦ìy™Ï?šQ¸w¯?ïÿPdè?'Ž5P ãŽ?Õóbýõ?'Ž5P ãÖ3FGL J2225.8+6045@Z"O~ÃT~@wàmòÀ9܋Ëz½6À:ò
kùM^¿òÎ?`"Â@ŸÓŸÏ¾š?ÿ&´Nߌ?éÅŠ†`¿í 4é옿ҸŠ©³¿Ãê­ÈГ×OTHERspp?ïù´®gJš?c|j.}8?I-FbՖ¼?c|j.}9?ï¨Â-}]? xšI•»?…Ït ¹¨¡? xšI•»?î¤[\ .ï?¢‡d¥ZŽ»?¥ºJ5ý?¢‡d¥ZŽ»?ïÿW;Aé? 7üúX?—Ý¢ä? 7üúl3FGL J2225.8-0454@M……rÀHj> N¿À8l'šÿÀ;g%ª´t?ñ2KÇ~¯3@F3´7€@Þl ¾4¿à>µÐ[øy¿æOEz³zk¿å€EØ|Xk¿êia1ëæAGNfsrq3C 446?ïð¯U8?\²ídCœ¬?_Øü¡U÷?\²ídCœ¶?îâä&m?´™æƒn?®¡Þ'½™(?´™æƒn?í‰ÃdT?¦m
‰ðs?·C±çäÝY?¦m
‰ðs?弫P"?¹qJ¡?Ԇ©_õÞù?¹qJ¡3FGL J2227.8+0040@Pw[À6ãÀFמ_Ñ÷¯À9'|üªàêÀ;"},{‰
?ñ±«®o@6Óü–ê@'?ØÝý?äÒ»Þ+ޚ¿å©`ã<¿â¤ØXŠõV¿ëÎQ":èAGNbllPMN J2227+0037?à\jŠÛ<?Ñ)ÝÁç?ßG+ÊêIˆ?Ñ)ÝÁç?Ü%SQ'¨k?Ñ^Úæ6I?áíVW6«Ê?Ñ^Úæ6I?Õ`{žý?º<@ñ€7?åOÿ}B0'?º<@ñ€7?ËÕf|+…f?²ÜqA±µˆ?é
¦`õ¦?²ÜqA±µ‡3FGL J2229.0+6114@Z© b
·@¡àE$¢À6,6*^x[À:tĪ¿[Ë@ž<ÓG:@'3DÐêi@&k×j¿Ø¼˜!I{Ê¿âêÚ»:¿åIÀÐó¬¿ì²Mx6{PSRPSRPSR J2229+6114?9ë¸oë Ó?9á‹B\î?ïüˆò‹?9á‹B\î?>qZ"R?SSu
%]O?ïü1Ô»¿w?SSu
%]O?"ÞÒéòÁæ?…ã—Ø×ð?ffl´X4ø?…ã—Ø×ô?&åµqI­?³À?˜*ø?ïÿ§di*:?³À?˜*ø3FGL J2229.7-0833@KíàBËWÀIÛÒÀ+ԚÀ7¤ä+Ž#À;Hª9$
ü?ùÐÁÙ©ª@‹ÆùÏq@©x3îD¿ä'ë‹îz
¿çggWÒú¹¿é7dQ캿íàP8bÙ$AGNFSRQPKS 2227-08?ïÞ0³€èÅ?jW«%¨P?pç¦?‹µ?jW«%¨F?ïïqPëe(?lèûÙÍs?`Ž¯šØý?lèûÙÍq?îyêԚn¥?šu¯
{O?¨aR¶YŒ?šu¯
{O?ïÃËä¾zÇ?|*ç#?~
 Âœá?|*ç#3FGL J2230.5-7817@st­••ÀB8H˒:À9Eg™TÀ;¤`·Ð¼À«]¥wžG@ؗýZ¬@P_"äN¿ç óäq¿å`Hü.u¿ãL
2ïý¿ë[×ãðï†AGNbcuPKS 2225-785?ïýô3NÓ?1ýI§ðÏ?0^gU‰k??1ýI§ðá?ïñwɂä?féËãAŒ?]lú7ÿè?féËãAŠ?ïj$ïêE?'{›ÁCî?'»"·>?'{›ÁCî?ïÿÿµÀg¹>¡Rµ5Ù>'æ{…è>¡Rµr3FGL J2230.6-4419@v³¿µÀLƒT_Ó¥.À:P/žS<¾À<V	!ò¿ã™õ&­ƒ@
ŽYõiÏ@"NàbÖº¿äÌRخǿèq‡DÓ¿Û9'Åö"¿í›oËÑ
…AGNfsrqPKS 2227-445?ïû³'—	È?DPs:ì"?A1¹£ØÙ0?DPs:ì?ïîZÔ&`l?l3˜šBŽ?a¥+ٟ' ?l3˜šB'?ï·öÁwß?'H'îÆR?ž)'Ñ?'H'îÆU?ïëß⇸?_îÕϳxÈ?d xGr"?_îÕϳxº3FGL J2232.5+1143@SZÀ5¯åÀCJ—à[õÊÀ7X‹÷§qÀ;#¾Šêª-?ü«zŒãþ˜@"HM÷"±@·'TU흿ãv-¨Ò*¿ç·@+T¿é¥*LbaÓ¿è‹隸ÓAGNFSRQCTA 102?ïô	:ùœ¶?XÝWÂ7?WíŠƓZ?XÝWÂ4?ïð0ó¡3\?g+y²½H?_ž½™IO?g+y²½J?î­À\R‹?ž:ë1ñ?¥#ú:ß·C?ž:ë1ñ?ïý¨Õ;¨	?9@L$*?2¹V"¿³8?9@L$]3FGL J2232.9-2021@Bºø_øŽÀLÙÌÿøsDÀ:A±Y©¿'À;ϳt62ÂÀG-BÖ¿@×3#žì@¥ùÿŠå!?Ç%£ø%M¿èFz™Šf\¿Ò_½m'Üj¿å+ñSAGNbcu1RXS J223249.5-202232?ïÿ%²qÚ? Å5«J£2?I±Ä¿­{? Å5«J£y?ïôûWãÅ[?cæ¸L?V	P8uM?cæ¸L?Fm?ƒŒ¦Øãç?‰ú.x$À?ƒŒ¦Øãæ?ïÿÀãú>I?í¤—4ßÖ>ÿŽàÛé?í¤—4àG3FGL J2233.5-1235@I&û?¦ÞüÀKR·?œÎÀ:N(´T0À;µŠª¡¿ü@Hð^Í@z}[‹a@û!_Ìr¿æk½à˜(¿à>Ó	Y)¿âR~WsÚB¿ãº#r AGNbcuPKS 2231-127?ïüºw¼?@I¼ƒ˜*¬?:,GZJÜ?@I¼ƒ˜*º?ïóa*M…`?d7@Ò­h?Y=«dõA?d7@Ò­j?ï5 oîI:?"ï8Õ¾•~?™Kò6ØÂ?"ï8Õ¾•|?ïÿ‰ó§t?Èw‡ÁŒ?
¸C"Çr?Èw‡Ál3FGL J2234.1-2655@9N¡¿ØȄÀMÂ'?ßéàÀ:êÛ«ŒáÀ;é"C÷¦•¿¸cðHà–@,¶Á™®@ÿ²}@¿è ‰	Ôj%¿à'<\kš¿äžª|.¾s¿×À<­Ò®AGNbcuPMN J2234-2656?ïú‹_':?WFsg!Œy?EҀõ·
?WFsg!Œ{?ïòú¨ùÜ*?dçí}DÒç?Z
®G¬Ü?dçí}DÒë?ïˆi³?‡é¹«L?å"?»üø?‡é¹«N?ïë+JàRì?\DN؍X?dÔµ­?\DN؍W3FGL J2234.8+0945@S "AÀD8G@0q¸À9"h¸P>À;ž
§ù®­?ú$ÉñP9Ô@ü¼(º´F?û¶\/Ö²T¿¿aÊ®Q¿Øý˜MY¿ç]RÑÅ@¿íò'³e6PSRPSRPSR J2234+0944?t
uG-ü}?vÙß%Z¡Ü?ï×åq¤?vÙß%Z¡Ü?·½ÛùSm?½RÉå>,À?íD€ßõ"?½RÉå>,À?™ÅÈ&>,<?'>­PÜÓÃ?ï1ѾΝ?'>­PÜÓÇ?³‡k1¨Î?0¹ïYb¸?íž/™Êæ?0¹ïYb¸3FGL J2235.3-4835@u‡É¥ÒÀL1@ìFÀ9?ÿxÃÑÀ;Ï3ÿáÍ?å©1°¸UX@·VƒÁ@æÄÀ8ê­¿áø4Tª°¿æp)Ý'¿ç­;)¡¹ú¿ïÿ§U¢|uAGNfsrqPKS 2232-488?ïÿUî˜?µý¸q?B>lýTX?µý¸=?ï°^;**7?Œ—€-Ú5,?ƒèq5urj?Œ—€-Ú5-?ï›>ÆÂÑg?ƒ±LÉPZ?‰0NOK¥·?ƒ±LÉPZ?íÿ0öâà? '"wi?°Hèý? '"wi3FGL J2235.6-2319@@.Vßà¥ÈÀM"
Ÿ–2ÝÀ9¥aÈqô9À;ÒaCöÈ?êô³JF†@ÐÎäÿô@‰¯ÀL‹Ê¿æÁd»ã½Ì¿ìm<<'x|¿ã@`óaK¿ï¯òuÝ
AGNbcuPMN J2236-2309?ïþT´µ?D5¯x¨?*´´®?	?D5¯x¨?ïڅLô7Þ?y4IB?r½Y…ä:?y4IB?ï%p±Ä?"tì·À?›QéÜ'w?"tì·À?íÖL°wÛÑ?¡§ªåÀh?±Mš|A!y?¡§ªåÀh3FGL J2236.0-3629@	tŸå
5ÀMöWŸúëÀ9lÙÑ.[À;Âßp=½?ܸA_r@á!c|ý@›ú¿Ï8b¿Û™`GØ«¿äø—'=J}¿ãêĊð¿¿ã4dœÈßAGNbllNVSS J223554-362901?ïÿœáOgN?
>rý{?Ǭ&,>?
>rþ|?ïîöW¡;?jH…Q?a	¨^ùÆ(?jH…S?ï¡‹»³?…1Ÿu'?‡¼9Óu?…1Ÿu-?ï³Í?v'΀Mò?ƒ"x–~?v'΀Mò3FGL J2236.0-1706@EÌ)ÿ­Ê©ÀLšŒ 4RîÀ:N×úþ8€À;ÓÂ¥+ž¿ôsÎq»@@å""@
3 "ÉK¿á™»&ÿj¦¿ÕTR|¿äÖǪ¿à"²k;|AGNfsrqPKS 2233-173?ïù<Grø?R× dæ²?Kâ6¢?R× dæ«?ïôÀ'
ï?`³ºy'ú?V~ûä à¬?`³ºy'ú?ïSPVDÀ?BpGþ(?••õ7|Çá?BpGþ(
?ïþ"C‡•p?'DJûÆM?&»Ç†©%?'DJûÆ)3FGL J2236.2-5049@uNß°Õ ÀK"î²ÑÀ:,M…>À;ã"q;¬~?֊Ø*ùÓÁ@
'ÇÍ3¤ó@ÚP (êZ¿áéÒ­˜¾¿æÜì/œ-{¿ëïée¿ïÿÝbh¢MAGNbcuSUMSS J223605-505521?ï÷AÊ} w?ViLk€?Q|k¿&?ViLk€?éޑ‡!Ow?ÆRëCcí?ȅ¹ãzÂ$?ÆRëCcí?î-,Œ ˆ›?œ)š"ޖ?­-7=÷ve?œ)š"ޖ?át²6n)|?»ãal¹ªi?Ý›"#­?»ãal¹ªi3FGL J2236.3+2829@V†à€øÀ9¢¬_nû`À7ÛAõmÕÆÀ;.ì³òá4?ø¤Z­ Œ¨@Çj²ÑN@5¸ÜU
¿à-Îy—'ü¿ãbºFÊ¿æ·£®à¿èæÜ­ë`6AGNbllB2 2234+28A?\)m?Ž•ð…ÖÓ?ŠÖhßµ¤Ô?Ž•ð…ÖÑ?ïá­qÁï?y]ü‡ýýî?nRŽ>ç?y]ü‡ýýì?쓳E=:¡?¨²ÊKe»y?»beÖ*ý?¨²ÊKe»z?ïùš¼}Ó/?Fýƒ•È?I•³F?Fýƒ•ÈQ3FGL J2236.5-1432@Gñû`^©ÀLßùÐ;À7y#zX‹²À:ÓÔÄ(?ø9ÕÙ滶@ VĹÜZ@#Ì:«¢†¿Û3T
ÑØX¿âQâǓ†¿äZÀþd,¿äØq*\yAGNBLLPKS 2233-148?ïõÏü&]?VèÖOؼq?T`ϳCÑ?VèÖOؼp?ïö"YQ¯…?a¦ð¥qd?R÷M\ õ²?a¦ð¥qd?î·îƒ5~?•õ¶âô÷?¤̨a?•õ¶âôù?ïÿüã<¡…>ŇvݲÊ1>¸æóÙ>Ňvݲح3FGL J2237.1-3921?âôÕ@"ÀMÌÿ ^¯¹À9§×ÂÊŒÀ;Íiϧr ¿ÙêÍ×lk—@APt6³›@ßß»<¿âCq"öO[¿äF†TËè¿ãèN.Ð稿á@ëæÿ(AGNfsrqNVSS J223708-392137?ïÿꑇÝ2>äY§–UQ˜>ånx"ÍÔí>äY§–US}?ïõÈëQ´@?bÈ·ƒá<ã?Tn)\—‹?bÈ·ƒá<å?ïફL´?sàßeÖï?oUTø³KÚ?sàßeÖë?ïÿà/ý>íbö…ºˆÏ>ïÐëø$x>íbö…º`3FGL J2238.4+5903@Z£h@[9â?ޝ¢ŸŸ›À7±E‡ÉÀ:²›ÉÂ@3¢x:yN@Wúÿ'?þsÆV;¿Ñ–·÷þ~Ì¿ãÈ´˜p¿çìÝÖVÛ¦¿ì›R[ÂsƒPSRPSRLAT PSR J2238+5903?<)ðÇo›?2ã²h^E?ïüzÁç?2ã²h^E?1ƒ%a$/?KùBpœB?ïýϝSÜ?KùBpœ@?wÇ,†è3¯?r@2Ù?ïÐq¦ò/™?r@2Ù?f;V
%™D?b 	'(?ïéÄ©òÚg?b 	'(3FGL J2240.9+5831@Z¥ƒÑF¿Â8ßowîÀ9•ÝŒ7±GÀ9›V	÷Ї?ú±¯ÀL‹Ê@¼%†¢F?ìêŒèé}¿Ïà'·)ø?»Za»¿ç	'6½›¿ïÿö¯Á›ŽPSRPSRPSR J2240+5832?ÌÝÅ^¨?Ïûm:_üò?ëûHŽ¨V?Ïûm:_üò?Рÿix†?Ôô÷@†ÿ:?節KwC½?Ôô÷@†ÿ:?¾É¹8ºd?®W‹€0®Ä?ì&ÈØè³}?®W‹€0®Ã?ÓVYV".?Ì,yüõç?æTÓsÔµé?Ì,yüõç3FGL J2240.9+4121@X‰}ßÿ¯xÀ.Oç_JHÀ:¿k»9ýÀ;|Î>½¿»x'b@敠¼@ž2 f<u¿ã\ûn¿ëT™¡ô~d¿Ôû¤åìÈ/¿á.»c\µ|AGNbllB3 2238+410?ïý?<9÷bz-è?7/o'Ük?<9÷bz-ì?ïÉS.wÅÇ?ˆÔv¯?{VhÄŒ?ˆÔv°?ï´¢Øqlÿ?€¡ÁßîM?'×Iã¤Àu?€¡ÁßîL?ïή¢ºAî?rR˜Ì¦£?x¨®¢ß	G?rR˜Ì¦£3FGL J2241.6-5237@u®6	ÀKuJÞ™À82ª§ÞÖ»À;ný`O@N\Õn@jt#"X?ü‰ïµ…'¿Ð©RÝ{#j¿Ö¦˜"Š'"¿âÚ°E‹-#¿î¸R‰åœ|PSRPSRPSR J2241-5236?y­<ë΄£?t¨w÷ò?ïÌ¥†(bø?t¨w÷ò?‡%Öº9/?Ž<úùª?ï£h¥«?Ž<úùª	?›ŠQlAËZ?Mù]Ìl)?ï#­tñ¤?Mù]Ìl(?aO#kÿê5?Zþãý6'?ïî°Ü"?Zþãý63FGL J2243.2-3933@vyÏÏÃøÀNW³ S\žÀ:eÄ¿¸TÀ;ð^VÀë~ù°/³@/B%¿W@ò«]ä¿ç—™‡jÿ¿ÝÆLM" ¿è¨šSd¿çj3;°tAGNbcuNVSS J224326-393353?ïÜæfM'?rBKÇGý?qŒÌÙ6þÚ?rBKÇGý?ïòø¾Û?fð\U/½C?ZäƒÐI!?fð\U/½H?î%zqyÖ?šýGxéÄ?­¯Xèb¥?šýGxéÄ?ïÿŸsЅô?UúÈÕp?#ނ÷¼?UúÈÕQ3FGL J2243.4-2541@<t/ ~û‰ÀN±W€•ÓÀ8¨Xçø¢>À;'Ì؋Fð?æƞ‰\Ny@ö˜Ô!Õ¾@2¹@(<¿á²Í¯m7Þ¿ãV'^o¿ä~v"T#¿ê‰2°Î¶ÔAGNbllPKS 2240-260?îdOñfÅ?­3ø½À?©»éŸó·?­3ø½À?ëâ{±j?Å%°Æ*7?Àv:UË?Å%°Æ*8?è3©U'÷?´Q!Z#?Ï£1Z«`%?´Q!Z#?åÆÅÍŽ=?ºƒ·-uÏc?Ôrteúã"?ºƒ·-uÏb3FGL J2243.6-1230@JRe?õ¹UÀL]â?û˜'À:%©|e¬,À;ÁÔ2Ûÿ?Ö®ãû	£@p-è±@ÀÊ+¿äG.B¼Ö¿ì¤"{ó¿¸Pí ‡èu¿ÖãlØ׃AGNbllRBS 1888?ïÿôà?NŒk¶'U?|ðõ›?NŒk¶'a?ïñԓ?h Ùä
ƒ?]ÊVÙÎå?h Ùä
ƒ‹?ï¿F˜vX¤?|Û-‹°Ès?€.YâiÖ÷?|Û-‹°Ès?ïÔ}öÙ\?p7âí@?uÁ"Qòø?p7âí>3FGL J2243.9+2021@U¥Â # –À@®(€QÉ÷À7³ŠÁéÀ:žoStò?òý>áß.@QŠDg
*?ü¢Ù;(ö¿Ö"÷ïÃÐW¿Ö'ÇɾᎿÙüÚkÆ̈́¿Õ¢/ÁIòùAGNbllRGB J2243+203?î·Wäo.?©>è©úcn?¤Š¹"?©>è©úcn?îåwìM7?ªóyw5Ø?¡§;,"?ªóyw5Ø?êx`
Q4½?«úÀ,8?ÆÖ»-
?«úÀ,7?åuûVvØí?ºj¼ið¤!?Õ	SN&?ºj¼ið¤!3FGL J2244.1+4057@XŸ£ÌhúÀ/"yÞé/À8¤zôŒÀ;?ÜìՁ?êÛBG'þ´@ë¸x¬äû@POŸ¥wH¿Ö¹k:p¿åT|/6µ…¿ã¶C¦üaC¿å'|/Œ›ÀAGNbllTXS 2241+406?ïú´¾Ê?DGtg«Ï?E-ŸôÕ?DGtg«à?ï×ó½\?gJ=•+7?t{¡R^?gJ=•+7?îØ«`1&?—5;
> í?¢uIüힻ?—5;
> ì?ïùÐMÛ	?@^rõÞ4?H¾ȓÜÙ?@^rõÞ<3FGL J2246.2+1547@Túâ€'،ÀBµâ (zÀ9•9"†À;<L$ˑ?çgØx@rP@Ùå_jÉ¢@v9à¡jô¿çy¯nm¿èû#½/²¿Ü'øª˜'Ô¿Í&hä3àqAGNbcuNVSS J224604+154437?ïÿqõúó²?ƒ™Ҍ?Á@¡‰°]?ƒ™Òu?ïîa2\0)?iʧ5×~l?ažÍ£Ï×o?iʧ5×~i?年ƒr( ?…0ît»ke?†\_#uø?…0ît»ke?ï¶	à´`?v§u1{?'}¿GÒèR?v§u1{3FGL J2246.7-5205@uFŸŒ!âÀKí: þ¡À:-¼ÎRÀ;ƒìŒ…´à¿Üœ²
™@
½Úg•œ?÷!ÀD(N?ïñA2œ¬Á¿Ý+$Ÿ$P ¿Õ~uh"EA¿³ÔꎺԎAGNbcuRBS 1895?ïþƒƒ÷Æ?)'ÁR:þ?'ÇÀ"È?)'ÁR;?ïô:@pô?dÍÎûQ÷n?W‹ü ?dÍÎûQ÷k?ïE‰ð3‰4?ÒÏAï|?—NÁùŽÙ?ÒÏAï}?ïü0Lá?8±ù<fp?>}ŸØ÷T§?8±ù<fG3FGL J2247.8+4413@Y-÷ µíÀ*€Ô`?ùÀ9¾P"–JZÀ;}ð·Ž?Ö$8'¨T@ "=¼Îþ?üºÊÿm3	¿ä‰?ðcˆ¿ÕŒ¤‰óÅp¿çxíztîÈ?ËÔÁÔiyAGNbllNVSS J224753+441317?ïn~Ic£u?"v+y?'06Ӌ'j?"v+y?ï½ ZEF?Š‰éÁ/"?€¿wén®X?Š‰éÁ/#?î]6GâÊ(?žÂöÁnE?ª,›Ó]‹?žÂöÁnG?ïԍ"rі?r‰")'?u¹nƗ4¯?r‰")3FGL J2248.6-3235@+}ÿ	_ûÀOué_ªŠƒÀ:ðôÊAØÀ;ñ9F¹?Μhv66@+渱7@"à{*n¿å´ŸzÀKÆ¿êD¼…Vìv¿ënL´cŸb¿ïýðõºÆAGNfsrqPKS 2245-328?ïúu³Ëe"?P¤-=Ìf?F)0Òiµf?P¤-=Ìf
?×Xj[?$þR5Qÿ?š
)åi?$þR5Qþ?ï`Ç)¥ßè?‡AŸìÅ.?"çËDÊ?‡AŸìÅ(?ì#¡N¾Í?¬îF*Ã1­?¿ÎâõŠ	'?¬îF*Ã1­3FGL J2250.1+3825@X²à'¤À2']ŒúÀ9(&¶ÂÀ;WD²·wÑ?Á½À´æ|@¬ƒd?þ˜¶?l§s¿å°6E®­I¿ßÁpïg'¿ÞóSãñ›¿Ö2t}xAGNbllB3 2247+381?ïÏh«ô?vŠ}öŸèf?xKöªq…—?vŠ}öŸèh?﨏œæ6?T*§ðy?…ÜÆy2z?T*§ðy?ïA²pMb…?'rG_+?—ɱöS¯K?'rG_.?ïuäOÅB?'îmü·TÑ?']cvW¦?'îmü·TÒ3FGL J2250.3-4206@v"Ÿ×¡<ÀN"¢¿³ÖÀ9½Ì'ãtÀ;À4"\B÷?éž©4'‹@³-QFï~@D– "Hr?î?Þù[\¿à5û×ý,'¿âžì>Ø¿èj'–qñàAGNbcuPMN J2250-4206?ïdÇo¤]?•»m9|4{?"gkt`?•»m9|4z?îëØ¿U}´?§&+Ò(?¡Bt
¨$Ä?§&+Ò(?ìՉ…K?ªoG]Ëݟ?¹S·¿›ÕŸ?ªoG]Ëݟ?é2͕}Â?²8PÔ¨ôÚ?˯4ɪö?²8PÔ¨ôÛ3FGL J2250.7-2806@7½f@¦¹=ÀO§¶€Z-sÀ7ÇtZÏYÀ;[^Ëgr?ï½icà"î@
Ő¡@k(_ššK¿àT¢pN¿¿âûØZœë¿ã õyÐa¾¿å¤ÓFíÿAGNbcuPMN J2250-2806?ïþ'qw?$ñ{¿²»ª?&Þh莻û?$ñ{¿²»¤?ïõPežY?`ÀUóçy?U_4ÂáK‰?`ÀUóç}?ï87w¬*M?'Wý]U]¦?˜ù
z¶ˆ?'Wý]U]©?ïýëO¬ÚÀ?/.ÓVó®?0¥'™)õá?/.ÓVób3FGL J2251.5-4928@uJ^`=WyÀLú`à¨.À9³C½Äò
À;¶V¼¥7]?îyù$]q9@©;"@?ÿx®àR»¿âzï(‹¿ÜSLÙ!š¿Ô§RR:èè¿ä%ržê!®AGNbcuSUMSS J225128-492912?ïã;‰uÏ?rtd½j¶?løÄvŠ3p?rtd½jµ?ï«Ê"Ù­?«bu?…
wIºO?«bu?î}Ç·p)?žH&ŒÎå?¨#ŽtˆýY?žH&ŒÎä?êÞºgÅJ+?ª'ÐTÔ<¢?ą`ê×M?ª'ÐTÔ<¡3FGL J2251.9+4031@Xè#¿ø¨ôÀ0àé_ªŠƒÀ9:$)ªô5À;‡Æßî¿ÓH:õR¸@Iá">éu@þh`f¿äÊD;œ<¿äW§¢¬ùÚ¿ÙéO¹?–¿éí'u¡ÓáAGNbllMG4 J225201+4030?ïÖ՛(Ñ]?| •ûv¨Ü?t•2k—Ql?| •ûv¨Ü?ïŒØ0R/?•½óBzá?ŒÉóë}4]?•½óBzá?ìŠyC£éC?¨"­ö‹Ø©?»¬5âàµâ?¨"­ö‹Ø¬?ïŬªg–Ì?t"MXWmý?})ªÌ4™
?t"MXWmÿ3FGL J2254.0+1608@U‡Å_ñ_ÀC_ÏspÀ4ƒJïèZÈÀ9ñ´Ï€t@7PÜfs@&LÉn¯?ÿ¢F…‰A¿áÀìªkV™¿ædˆ­ZŽ
¿æ˽ eí¿ë§òX*A%AGNFSRQ3C 454.3?佷ۗpý?ÐX‹ÁŽp?քHÑ?ÐX‹ÁŽq?ïì6£O,?y‡Ló€3?cùÉ\°Ô_?y‡Ló€3?ãEçÉ.@ˆ?»"€mªt?Ùt0m£~ð?»"€mªt?ïÿÿg¢XV>º*AèÿƔ>"´õ$«×>º*Aèÿ»13FGL J2254.0+1403@U'‹ŸÛÒúÀCõrØœÀ:0<îÀ;aC§õ|ï¿àõÖã?ïž@Uö÷Îÿ@ì‹àžeÜ¿æ4»ÚåÄ¿èÖN+î+¨¿áô%öø¬¿É#ò)ŽÖAGNbllNVSS J225354+140439?ïÿÄq¡È?LÊ*ÝúÏ>ýÇr/}0?LÊ*Ýû,?ïóÌ&=ך?b'F:ۏ?Xg³"PÌË?b'F:ۑ?ïÂäú•þ×?|¼X
E¹?~'µ"¸?|¼X
E¸?ïýÌ9æü€?.eÅÕܧÒ?1ž0Èø.?.eÅÕܨ63FGL J2255.1+2411@Væ æÀ?ƒ:€.Ž‰À9_h-æÃÀ;€·Á¢Í¿Ób:h—Õ0@Œ—[Pޕ@'ž‡t©¿Þ€ÔñßUæ¿ÏÁô—1›¿æ:'Dˆ¿Ú™ó¿ˆt6AGNbllMG3 J225517+2409?ïøÅ¢o^?R¦ˆ[QÞ?Léw¾BŒ«?R¦ˆ[Qè?ïí™æŒ
$?kñ1v%Ÿ4?bfsòÛÊ?kñ1v%Ÿ7?îqø"h€?¤(|-\o?¨àw¿™wù?¤(|-\p?ïúiQ˜8™?B"á\…NP?FZ¹Ÿ›È?B"á\…NU3FGL J2256.7-1022@M›Ö_ó…žÀMCÀI0ËÀ9˜OYÚféÀ;à,/2ór?ü
߬ùH@¸åå!­?ùrLK:\?íN'˜Œ¿×lôS¾1î¿æ&äv?U¿íšpÙÃPSRPSRPSR J2256-1024?P ·ÑU¤ð?X¹Þê¤Ì:?ï÷ï¤U.?X¹Þê¤Ì9?u_MÐÙ? ²©‡?ï|Um'z? ²©‡?±îañÁ ?¥Êt¾ÏˆÅ?íÂ3ÜáÇÜ?¥Êt¾ÏˆÄ?v}f".ÿ­?lx£þÅGB?ïÓ2÷¢?lx£þÅGA3FGL J2256.7-2011@DÈL€SÀOt?Àà0À9HÄIpŒZÀ;—¢çöô¿¿âíÐ.q~@
/óf¿|­@½}ÿµ,r¿Ý}Ì¢8,J¿ã[úk…¿ßp÷TñÛ
¿ä¹±~AGNbllPKS 2254-204?ïÕ®ø[{?"OŸñ?u(ƒÒvÂ~?"OŸñ?ïÎÉ'	Pw?‹˜§¶Ž?x›l{WÄï?‹˜§¶Ž?îMétt?ž÷¸ëâ?«!n¯8¸Î?ž÷¸ëâ?ï'ìgåˆù?‡<)údBE?DæÁâ?‡<)údBE3FGL J2258.0-2759@8ZÝßCÇÖÀP:B×P´À7¾Éãä@‡À;=ĵ§Z@'ûE[(ñ@Þ%™Â‰R@øӞM2Ž¿à¾o'Þ9\¿æ—ò_®fZ¿ç:c‡Jë¿íD¿ÇžPAGNfsrqPKS 2255-282?ïÕ¶5Â?puŠð2»?us¤ñeÌ?puŠð2½?ïòÔ?fuZªw?[ãÒWÝÎI?fuZªwŽ?í;	'Ó­Ž?¦(­¾Ûz_?¶'³éb"—?¦(­¾Ûz`?ïÙøÅÿ/?w¨.»?!'?sôi?w¨.»?!…3FGL J2258.1-8248@s04ÿ†]}À@³€ KÏâÀ9‹pd*À;vx†?Ò±ó¸Ê@ÏZs@ŒóŸŸm¿£q³üª¿áÙþú±7¿à&Ì¢Qñ\¿èUj3`»¾AGNbcuPMN J2258-8246?ïàýçŠ&?r³—uh—?ouäڔ?r³—uh"?ïÈwUª6Ò?"6¨¿w¹§?{ÄU*ä–X?"6¨¿w¹©?í¤ôNý‡‡?¤ÐL"ƒ	?²Ø]ˆÃÉ?¤ÐL"ƒ	
?îëÁ~—?ˆÇèaÏd˜?¡Cæ/8?ˆÇèaÏd—3FGL J2258.3-5526@t®÷_²íþÀK'¡ ÏÀ:zi
à"SÀ<ë7@?ÑòG" S@Ò3>íÂ@|®¸'¿æŒà/¿ç[î¤ý"°¿éÝ=K˜?»°fQvHAGNbllPMN J2258-5526?ïÄý1î3C?†w#®°Ð?}gæ^Ö?†w#®°Ñ?ïò¿	ãm?fgHtÐ?ZíÈ9(!?fgHtÊ?îPìZI³ž?¢qJ§lôS?ªñ:[dÆ?¢qJ§lôT?ï¹Þfä¢È?yÎf™¤Ö?ˆfF×N?yÎf™¤Ö3FGL J2300.3+3136@X5 "ÚÀ9
¿v¢õÀ9Eˍ1¬JÀ;df\Ukl?òˆ–i¹W$@¯¼EÀÿ?ý™ž>ÄáÇ¿ãŸM›lC¿Ì-H"÷Ò¿Õ-	²u!"¿ã~bª€WåAGNbllNVSS J230022+313703?ï²¢Ýþ?Œ•D\ÙR¤?ƒWy€R?Œ•D\ÙR£?ï^*úÒbñ?ž0láG÷?": ¥³¡Ù?ž0láGø?íM´§T¿?¦q£zðë(?µ'ZÅZþ?¦q£zðë)?ëÿºøp?ªiã›×h´?ä½>?ªiã›×h´3FGL J2301.2+5853@[Fú>¯h¿ï'DŸÀ9Á¾òïvEÀ;:9%»{l?ò³ç®O‰*@åÆî¼a?ø7¥þ׶á¿Öæê…Dwÿ?ïþzÄÂ<P¿ØŸa´ü¿×Á›@bÇOTHERsnrCTB 109?ét,¡ÿü?ÂvÓó‰ù ?Ê/Mxœ?ÂvÓó‰ù ?Ü
ù6UŠ?Ö\é9L'7?áúƒdÕs:?Ö\é9L'7?é³×¶ß¡¨?¯£…ˆ+7·?É0¡$y\?¯£…ˆ+7¸?äâ¨/¾?À¸'TQî*?Ö:¯Õû ?À¸'TQî*3FGL J2302.7+4443@YÙN wmÀ+ù¿è,À7ý£ª"" À;L(T²ß¼@-ù압@h´Is<?ú'òg»ü¿©ÿP¶.ƒT¿×ÿ'¶•B¿âs~õõ¿ìß²ÔPSRPSRPSR J2302+4442?`dIgæ?ZÿdW¹{?ïó˜è?ZÿdW¹{?q¥Ö¸?š±tþçq?ïÜ´àSæ'?š±tþçr?‡3²ê‹)%?ƒvæRñà?ï£14UÓ\?ƒvæRñÝ?FÙWLvy¾?B¥¹W<™ª?ïúIª,âb?B¥¹W<™ª3FGL J2304.6+3704@Y^"ñÀ5"ÿÖåUÀ9q¬'$ZÀ;iQÝBeÖ?Ýí¾jŁæ@¤Ô…'ò?ýÀŸ¿äm½å ¥Ÿ¿çÇ"5¿ÌèZ²Ì¿²<´fN"ŒAGNbll1RXS J230437.1+370506?ïý¶î×¹•?<EŸ£MG?2H‰B3Su?<EŸ£MT?ïݦ'¦C5?zÿéíƁ?q,·,Þeé?zÿéíƄ?ïËk™ÅDò?~œ#o‰MÅ?zJ3]†V?~œ#o‰MÃ?ïô6³1Ù?P¸ýÑ/ ?Wý'™œKÉ?P¸ýÑ/›3FGL J2305.3-4219@uîCÀ~à±ÀOÎ*ŸæºµÀ:ßNG‹¯ÌÀ<]û]Ùпê/wAÞzR@
¹µ.Ëo€@b¿g£¿í ›:¥å¥¿ /-¥ l¿åoº 9¿Ú]2p?®AGNbcuSUMSS J230512-421859?ïô\¥t	b?dCWÆ@þ?WFµí:ü?dCWÆ@þ?ïò¢¸ÌWO?f[cKC—²?ZºŽgQek?f[cKC—²?îÍ'ô•Ü?š2¤۞î?£-€¶®¢^?š2¤۞î?ïù\1pžÿ?F$Ôlÿɶ?J:="š?F$Ôlÿɱ3FGL J2307.4-1208@Mµ?Àà0ÀN±v_Ø­¬À:‡kþUÛÕÀ;Ç%l¡¿Üø'y'Å@q!Ôæ÷›?üXFÀ®±Y?è@wO€¿åFðqdÆ¿èC,f ¬"?áQoß6öAGNbll1RXS J230722.5-120520?ïõ@y'ê£?^bÒÏw??Uú*¶
?^bÒÏw0?ïótvú?dZÖbHš?YÅöp?dZÖbH?íqKkÔr?¤irºÚô?´u£"¡\f?¤irºÚó?ï÷´kŠOÏ?VÀ¢¬B†?P—(ë`aà?VÀ¢¬BŒ3FGL J2307.7+1449@V5X`fÀDŠæü9¢À9ñÝ'ŽÀ;gÝX5K;?Ï$¢v·íB@lÏ$ÀԜ@èj#ç;¿â}ˆŠ¿â˜@URb¿ä¾Æ³>lˆ¿Û³ÝF[rÜAGNbllMG1 J230734+1449?ï¸ï
î'h?'æÙ¶š^H?Ä<"v&?'æÙ¶š^I?ïܙ…A""?~¸ܝº?q³=_=ïÅ?~¸ܝº?í2e×K¡?ªMÚ/ÄÞq?·ælÑE¢í?ªMÚ/ÄÞt?îÑDqÞ¾V?"ùÉpó.Í?¢ë¸â¬?"ùÉpó.Ì3FGL J2309.6-3633@Cï@j(hÀP ½_ÜßjÀ9øÀysžÀ;­›÷Aë]¿ñsCÄzï@]¸šºx?ý«¢¥é¿é«FuÔG¿âÚ2ÚKæ¿Éð'ék¿âD.ŒÊ*AGNbcu1RXS J230940.6-363241?ïÿ²¨_àÐ?rW<W¢?Uèˋ?rW<W£?ïô]Êߖ?de›';À?WEÒj@ÒÈ?de›';¿ý?ïÚJJÛ©>?q-1ù÷ò?rÚڒ+`â?q-1ù÷ò?ïÿqø*?Žçl'áß?Àú¾}À?Žçl'â(3FGL J2311.0+3425@YPaAcxÀ8_€™"À7‹áP°À;&ûL<µ?ûz9.Êó@3¼]éÀ#@㶿á™üL[7¿åWʯï¤ò¿åY‡lÀV¿ëÌkŸÐRAGNFSRQB2 2308+34?ï¡( •R@?…6¾×ÿ(?‡µ÷Ú«p<?…6¾×ÿ)?ïçY/B?r‹—úh¥ÿ?h¦Ð~€¾?r‹—úh¦?ìÃG1Å@?¦ÈtE<Æ?¹ç…ÆqÕô?¦ÈtE<Æ?ïÿpËÄFR?Ý÷ˆ‹	²?æ‡w5æ¸?Ý÷ˆ‹
±3FGL J2311.0+0204@SÔúÿåþÍÀJ
@TƒæÀ9ÜàáVǍÀ;Æ)}§ËŒ¿ô
ý\aªÀ@d¿o—ª@+b€R˪¿Àâô:"¾}¿æÕÝCßË$¿æ˜	Œú¿Ï¯7¼AGNbllNVSS J231101+020504?ïýA§ör?:ªÏ™0f?7-òÀLm=?:ªÏ™0‡?ïó&°™{?f‡Ñ=Ob¶?Y³ÌžÍP?f‡Ñ=Obº?îúÚ`?–Úè‰õºZ? ^OßÒYþ?–Úè‰õºZ?ïÿ½sâ?û~°ôŸŸ?¿ÿ£¦ö?û~°ô 33FGL J2312.9-6923@s¯£¿ø¨ôÀF®v?ø="À:Ë-œ}ZÀ<	،°?ã›U"Iƒà@
^,±
ÿ?üÝK?nå¿ïÿù?Ð??ïþÔè‹Uo¿°œ§W¿ä8tƒ4¨SAGNbcuSUMSS J231347-692332?ïúrt1žÖ?L÷Ӗ<³?F6/9"©&?L÷Ӗ<£?ï²è§¸Ær?l½¥H`8?ƒEÖÎc›?l½¥H`8?ïP«Ü¤ÓÚ?ŒÖl¿<c?•ê"ke"Ê?ŒÖl¿<f?îvÖygô—?¦£•6ˆß?¨'˜i€¶‹?¦£•6ˆß3FGL J2314.0+1443@V¡ùŸÿhÀD÷"ßÎ1QÀ9Ž—rwì¡À;f"Ú<ø¿ðÃðBÛ@Ýá"êµì?ü \†ã‰¿'îâ:6 '¿Ôa÷8R¤¿ßï§yu¿¥Šòóä$AGNbllRGB J2313+147?ïíý"^?j_epþ£?bl¡îéß?j_epþ¦?ïòŠÚßmj?d°((éJ?ZêJA%*Þ?d°((éF?ï Ã÷Ê-=?'¨Aq†[p?›çºXn?'¨Aq†[r?ïþž¸FÈ?'xðû>%-?&{"~Q?'xðû>%h3FGL J2315.7-5018@tê ßÞøHÀNAY@
6IÀ9»˜"à5À;Êd¨ E?å1®v©S@
ÀXr‡ÜÙ@†@.l?ï+šeÏñ"¿ÞtXÔ¤ÔÙ¿åmÊ"Dñ¿ëÒºŠUAGNbllPKS 2312-505?Õ¢W
LU?È»"kú…²?å.õÔyYÕ?È»"kú…²?ä8lûfµ?Ñx.š‰}'?׏&	3ð—?Ñx.š‰}'?äyé3•t?¸:ù–À?×-˜Õý?¸:ù–Á?Þ¾Ÿª{H?½Ðƒ·•´?à °*þÂ\?½Ðƒ·•´3FGL J2316.8-5209@t¼]ÿÅGÀM«t`$-À:£\ŸTÀ;ޏ±¹K¿è i6ÐK²@jîªB3V?ûÂ@&¿èó(!öñ¿å
m*È"¿Æ<C_½r¿Ö§kŸ‹KAGNbcuSUMSS J231701-521003?ïÿÃ\Á?A°Ãm8K>þQÿqñ¢?A°Ãm9æ?ïôkÀŒ¥¯?a±:eB3ž?W(~æ´ -?a±:eB3?ïÓ2¥ÐpÐ?wºßÍ©	?vf­Ǘ¬?wºßÍ©
?ïý~Òa¥?3'–´A?4ylòØ{?3'–´3FGL J2317.3-4534@ua›«–òÀOà§`+¹ÂÀ9kÝ3L]§À;²ýî­È¿Ê$Û
ŸÀ@â%¯çä«@}1ÿò¿å"¸#G'Ë¿ä5wãˆÈ]¿×iØM€Þ¯¿åD;8?SAGNbcu1RXS J231733.0-453348?ïÿ_)•Æ9?R°ÕÞ(?ÍG8âò?R°ÕÝÁ?ïîâ(p?gNÌh'þÝ?a׏ûÿ+?gNÌh'þÝ?ï̂ÒúÆ?~ÇDw'?y¾–'œü?~ÇDw€?ïäӎ•û?bû€P$Z‡?k,qjáû?bû€P$Z"3FGL J2318.6+1912@W£?ãDÞÀC?N™À9ÍS¿šµÀ;´¢Þ¼¹Y?à}Ç2÷v@	(ô@P@íÊà
œK¿èǚ´Tc¿èMÎɍc¿èúœQÀù¿ïþŸûˆwAGNbcuTXS 2315+189?ïì—ó‡ã?kù¿÷ ñ?chýx­?kù¿÷ ñ?îUMé£øâ?´"ã}''?ª«!eÀqØ?´"ã}''?îÍ5/ív??˜02-²?£,­(œ
?˜02-®?éj
)¹«?³î¹<*B?ˊW×YW?³î¹<*B3FGL J2319.2-4207@uÆ# ƒ˜¦ÀP|Ù ,Æ2À:7_èžÀ;âØ+¥ 8¿çG²,s¸@g0¨êD'@¾àP]¿Ó&(;f3¿æ,u
Ü¿ß|c0"ŠÇ¿Õ?\hØþ×AGNbllPKS 2316-423?ïþšÆHoK?3J"ð[Éø?&S›yY^?3J"ð[Éê?ïò¤e1©ì?g"Èà¼È?Z·5œ¬&†?g"Èà¼Å?p°õ?"ÈÍñꋿ?ˆÜãüÃV?"ÈÍñê‹Ã?ïû•˜fþ?:ÉG%A?A©žd›?:ÉG%@À3FGL J2321.2-6439@sځ¿½ð'ÀHç( 2:À:ªößÅÍÕÀ<	ø¶_¢þ?Ù+ÿY´H¿@'¨ÀSÓ@4ôBp¿é§ÇQ/?¿çªyW@¿Ùù¼ÚçB¿á>ãAAGNbcuPMN J2321-6438?ïüªýƒŸ?I5
F9™,?:¨ãň?I5
F9™5?ïéY‡«%?qŠªo—µ?f¦xTÚþ.?qŠªo—¸?ï5Æáh-i?–«Å֑k‡?™G#ÒúS?–«Å֑k‡?ïQÆêdߣ?Š÷Œ—Ž>,?•Ç"³d¡?Š÷Œ—Ž>+3FGL J2321.6+4438@Z¤[0HÀ.»›>µGuÀ:ýþž1À;ºÏ' =¿ÚRqÿn,%@k¢Câ-@ÿYfú¿ç¯3ëáæ¿ì8æv1Æ¿ÛId祿ïÿŽî½AGNfsrqB3 2319+444?ïþÜöŠz`?0Š6îv¿?"0—XZ"?0Š6îv×?ïŸfSÞ@ò?'Å5!ó¹¾?ˆ&koÃÇ?'Å5!ó¹½?ï-"Í?ÑF?'.;½?šM†X×O?'.;¼?ïÑü'¬ï?påöú¤?w¶ñ)ˆ¶?påöú£3FGL J2321.9+2732@Xêãÿï9À?A§¿Í
	À9bCá× 
À;¢d¾£À	/]k!Ð@Hÿnàˆk@BPàW`¿å']竏)¿â's%Ui¿ã˜|+RFÒ¿â	&I{RAGNfsrq4C +27.50?ïóW/¦?YÓ¿."ž?YQ ³Ûøj?YÓ¿."£?ïïpOO÷P?lnäæ*É?`°°°!?lnäæ*É?î…~m›É)?š"ýÁ".?§¨&Cme?š"ýÁ".?ïÿîg§d>ö·vp#â_>áê˜Xš¦>ö·vp#âí3FGL J2321.9+3204@YkìAÝ"À;àÿ‰¸{À8«ˆTüÀ;j´MzV?öØïæ|,@9DQáõ@,n;òÊb¿Ø›£¯¿ä%:cËxÜ¿ä˜1&éxÕ¿é,ÛGÁœAGNfsrqB2 2319+31?ïÎ|®gó?}›KÇÄþ?xÁ¨Ì}‡®?}›KÇÄÿ?ïâü4rþ[?uGÞõsâ?mˍ£µ?uGÞõsÞ?ê°ãpX+G?°(¹]*Ú?Å<r>ŸRã?°(¹]*Û?ïð»+†r?X3[c"X?^‰¨Þó³?X3[c"S3FGL J2322.5+3436@Y·ÃŸý`éÀ8ÇóÀVœÅÀ9þæªÄdHÀ;v zÉʺ?çS¬#xÄÒ@"DvÒoN?÷­ µT?Ñi-竹¿êAb7­–¿ÐE­e¡¿'ãžSbAGNbllTXS 2320+343?ïç§Û(©?uåc-aûd?häX$×VA?uåc-aûf?ïÕN$ã;Y?{ƏÿÀ¨?uXíŽbSâ?{ƏÿÀ¤?î¾9ÔÚj¢?šq§†Ìßt?¤b²YUÞ?šq§†Ìßq?îÜa‰š(?šÙq0Mï?¢9îGf]{?šÙq0Mî3FGL J2322.9-4917@tè¶@c^ÀOÏ`%ÆÀ9Ïûf=K»À;¨Ø+¥ 8?æD`ؐ'ø@lõÌ ?ÿPý Q¯?ïýÆÖØX5¿à'ÞIvìq¿ß̃ˆ©¿âOuiõ£AAGNbcuSUMSS J232254-491629?ïô¼Ñ•q?ZÎwC¾Ý`?V†]èÕ"?ZÎwC¾Ýg?ï¿Ý]8VÉ?…äk+ÿNø?€¨±êMû?…äk+ÿNö?îÒ*ñíz×?—fÁ€;Ï?¢ÝPá(R?—fÁ€;Ï?ëÏòšCÃ?¨ÄX|}G?ÀÀ5½–ðò?¨ÄX|}G3FGL J2323.4+5849@[ïÆÁ#À3€5'À7Á»øi3À:™MüUy?þœlâ×P@
†"Gwã¼?ñ'‹h(ˆ_?ïÿeÛüëy¿Ë¢:§ñ¡¿Øh|U»ô7¿á—"¤%OTHERsnrCas A?â@lNÄj?ËY…ä?ÛÝ'bw*?ËY…ä?Qú=K è?i]úBW'±?ï÷áZoô?i]úBW'±?⬒¼Ìü?¸PîOD*?ڦڇîf
?¸PîOD*?"xb'q@0?†Öt4[cl?ïd<ëìuÿ?†Öt4[cl3FGL J2323.5-0315@Sr‹`òËÀM@TƒæÀ8,ë-
$FÀ;K_Û1ê^?õðÚmÊ2ê@©8<²bé@}8ßðk¿ßû²WDy¿åÖhãªp¿äƒcþ"T—¿éN,™¢9AGNfsrqPKS 2320-035?ïã¹ßoN?£–ªý~AÓ?lF ±íá?£–ªý~AÓ?ïó€ËlÇÜ?b@=å‹?Xþi&pF¿?b@=å‹?î›*›%?¡gŽ8–q"?¯6OýVM²?¡gŽ8–q…?ïÕ=Qº#?pÆ3
Ÿ»Ö?uap×"îÄ?pÆ3
Ÿ»Ø3FGL J2323.9+4211@Z"º@Ù$À1Îÿ:cÀ8—nVõ°À;&Lké]&?Ñ32á0:@òÏ1+7?þ3'€ù9½¿âVÊÚóñ¿Û6fã}­¿Ü?_|ùa¿Õ¬HßÂÉAGNbll1ES 2321+419?ïÿ+PÃ%[?óƒ*Ž"?•ç›T¯m?óƒ*e?ïÉz"V¢¢?…Åä² q?{B½Ô®¯p?…Åä² q?ï̪§~B!?|vœSü	?yª¬@Þðá?|vœSü?ï÷'i	õ?F"öÈuýß?Pûõ-ì[?F"öÈuýæ3FGL J2324.7-4040@uãV¿Ê…ËÀPå}ßÿ¯xÀ8´@éÕPÀ;
®J*Æ?ë<¶ÅrÍ@
Å6ϟåä?ü*@›P©¿æ•¡%ª	¿Ó~ÉDé$¿ÕN›}ÁÄ¿Ô],bAGNbll1ES 2322-409?ïºvè¾W8?#=­Åƒ<?bEÐj2?#=­Åƒ<?ïÉwFL ?ƒá@‰4 ?{D{ÜÙ°H?ƒá@‰4Ÿ?í¿—š{™?ŸûÃ
C?²C/<#7?ŸûÃ
C?ê:ä¾r´1?±\w6Â÷?Çm5/9?±\w6Â÷3FGL J2324.7+0801@VA©¿ìêzÀH†|à%o%À9];÷'À;*Ž:Á¿úÖMI^î£@/Ø;Ù@5æzyC¿ÄT‰ Žfœ¿æ¶à'>祿ÝQ"	ve¿àGBAGNbllPMN J2324+0801?ïÿ«2—Ï?
²ÍÛ7¶?3Z:ŒhÖ?
²ÍÛ7ß?ïôêöZ¦7?c¡ka‡?V*J³'2?c¡ka?ïÈCfÍ®?5Ý5ö?{ÞqL™(?5Ý5ö?ïÿàzˆ>óDÙ0K¢¡>ïæ…þwó>óDÙ0K¡ç3FGL J2325.2+3957@Z`u>p~À3ûý€É¾ûÀ8ñ?Ãdn?À;^>¢‹±?øž|DŸ[@—ò'OOI?øœcÎ[˜?ÇñÃ.ñã¿àzµäå¿Þ´3ôNF	¿å¾ÄŒó$AGNbllB3 2322+396?ï؀¶'5Ù?fs]`^?s¿¤·ey?fs]``?}‹P±?—/¾²?‹ +ӟ?—/¾²?ìñ…W?«é‡]ܨ?¿ØsãÕH?«é‡]ܨ?îî IÁ"?}
8«6f?¡ûg#íÍ?}
8«6f3FGL J2325.3-3557?ý"YßDs¢ÀQmœýç!À8¾¨C€ˆQÀ;‹³ünñ?üÑÞú¡Ç;@­¶Ð·?þ'Ø	kä¿Ö¸§'(¿ãpPJU¿äÉHROX¿ïÿæNËaŠAGNfsrqCTS 0490?ï;¥wxsi?Ü)*Í?˜‹Qñ'è?Ü)*Í?eéh†?"â"â¾?€ž…¥ÞÈ?"â"â¿?æi³'ë>?³öj_õv…?Ó-˜Ü)…?³öj_õv…?îœ
n¦?¦fœZ™¥¿?¯Æ?Yžä?¦fœZ™¥¿3FGL J2325.4-4758@tÿ¹ÿÖ•ÀO¡ƒ_›q
À8÷.=*,úÀ;wv¡G
¿ÂÌV|°Í@CDÁ{
@|| 9›Ø¿â®Øê,¿éêï¼TÉ¿àŠj%™í¿Þh¶ª÷eAGNbllPKS 2322-482?ïÿìáY8>äP¿è˜![>〦È*Æ>äP¿è˜#?ïôi.ê™]?d–2ì,6?W-¢*ÍIE?d–2ì,9?ïÚi%òÇß?sDÉb¼'S?rËmœr?sDÉb¼'L?ï÷Û} 6?EOâYÙ?PIÅ¿'Ä?EOâYÔ3FGL J2325.6+1650@Wɪàú¯ÀD®ö@c^À:02ˆéH.À;ÙÏsëŠ?ҏ‹Ž>Å@ÎÙçè\@Ï\ÿµWe¿×C[Òí*ï¿â.¼Á'ۿߊ‰|§+º¿Ü	¯j«qAGNbllNVSS J232538+164641?ïÿ\Òoè?Ïl_qÐ?e²ÿ¿´?Ïl_qÏÔ?ïðt†ŒÃ?d¡¹(¥É›?_òçâ|€?d¡¹(¥Éž?ﱄ
8C–?ƒÎ,á-Û?ƒžýqïw?ƒÎ,á-Û?ïä¸{Ù
?[ëi!².?kâG"&õ´?[ëi!²23FGL J2327.7+0941@VÎ]ÿú÷ƒÀGûæ Zé[À8sþk«IÅÀ;Sï«&\?êê+žQ @uiäu5@lÆ 5T¡¿ç',ÐÔªx¿çž¯rô¿/¿ìûXùé¿ÔHæ"¥AGNfsrqPKS 2325+093?ïÿB›B³?!è4‹ž?w¬—©¥²?!è4‹®?ïóáúSó?fªI÷¸»Z?X=ÒX\?fªI÷¸»P?ï
mP»Žÿ?"ºŸ©)?ž²UèŽ ?"ºŸ©)?ïþ'Ælg?',ŽhMÉw?&ә>9€+?',ŽhMÉ`3FGL J2328.4-4034@u×TߋrÀQJërªÀ8r2$?ziÀ;M=5´Ã?ï¹+è'#~@Ïz>üë@wö?ŒÝɿݵÓ€ná¿çñ@/׿ã¥'¹ßü¿ç{$Ö³šAGNbcuPKS 2325-408?ïþÍRa"?$aáÞ5¤L?#*ß	çϖ?$aáÞ5¤ ?ïõ¦70}(?aäÀ¼±[?T³'Ÿ¯I?aäÀ¼±V?'ú?"0?ëá£?,«;©?"0?ëá¤?ïû¶}Ž??;'&Ðþ?Cå&½Ë¶??;'&Ð#3FGL J2329.2+3754@Zb'!%¶À6*ÅÑqwÀ9^'åp1ÁÀ;rùÒ¿U¿±Ž7°ñO
@Êt[òo?þÖϟåãõ¿ÚY^ÅLÄ¿æèϼý]¿ÓœÎùÁ¢¿ÉËV=ô?AGNbllNVSS J232914+375414?ïü¦i'[‰?;æYtšj?:̳u#¼W?;æYtšj?ïàÒ±^?zÅU^%-?o-N¡ñò!?zÅU^%.?ï²ÞM‰À?q~8fBò?ƒHx,?q~8fBñ?ïó¾$}bþ?L•È"+?Xƒ·:¥?L•È"63FGL J2329.3-4955@tÀ@%NÀO(?ßéàÀ6¢áÌ8RWÀ:Ë%Ü2›@Ñ´d ;	@ ft"§lk@…ž†"W‹¿à®•ó­óT¿äâSþô¿æ|ÖJ­€à¿ê(…	¿œAGNfsrqPKS 2326-502?ïªfˆe>›?†¼2D?…f]æ°Y?†¼2D?ïõfû¡À~?c²'k#ò÷?U2¼ ?c²'k#òù?ëN¾°M?¯Õ¯~"ø?ÂÇë‰>Ì?¯Õ¯~"ö?ïÿ™?2Ù?Œ­bBc?	°3zI€¡?Œ­bA¡3FGL J2329.9-4734@t÷:ÿ°NèÀP_¿î—ùÀ:*Jmâ\À;½êi•ÅÐÀq—:ï•$@Á3¼p@Úf€'ŒŠ¿ãýß-;f¿Ü•AþÓ¿è÷%L¯tç¿Ë™ˆ/lˆAGNfsrqPKS 2326-477?ïçÞ¯zÅ?ná҅ì"?h!P…ý:ü?ná҅ì?ïõ…GÁ»}?b†E8ÿ¹Ä?Tõp|‰%?b†E8ÿ¹Â?î'ñ¯ò/¥?œ'ÒMX?¦Ðåݬ?œ'ÒMV?ïÿèTÌ\Ñ>ïmâtÓ>ç«3£.û¨>ïmâpò3FGL J2330.4-3726@vJÓß°Õ ÀQ"ÓÀíÀ:TX¸þ¹¯À;öBzÎÓ7¿à²$'( @*éÓmо@Ž€¢§µ¿ã/Bóçæ¿ã8ßi nÏ¿æȹz¿áÁÁ¯@—AGNbllPKS 2327-376?ïö@SiwÓ?Zg¹U½BÝ?SY-[^?Zg¹U½BÚ?ïóEÁ1à/?b⤊}k?Yt}œ?Ÿ?b⤊}m?ï>Ö)áX?'gî¥F¾¢?œ%:ÃÔß?'gî¥F¾ ?ïëïloÎ?ZÛ)«VÅÛ?db"0é?ZÛ)«VÅâ3FGL J2330.5+1104@WD¶ŸÏ=ÀÀG†"`LpòÀ9¦5\_VÀ;‹võ)ã(?ÅÚ­Âè¿¿@|û£$ð@p¯Àw~è¿æV< Õ^¿çüŠ I¿é	¶™üã7¿àpý~ÎðœAGNfsrq4C +10.73?ïýQ`LÎc?6ùî&ƌV?5tý™Œðÿ?6ùî&ƌJ?ïî\ûªŒI?nlo
x©'?a£Us¶A?nlo
x©*?ï®{<b3?EŒE3ݖ?"a;0çsP?EŒE3ݖ?ïŽ/‡_W?}å­¯Í?Œt(<*r?}å­¯Í3FGL J2330.8-2144@FtqŸÀQº ÒH7À8é¦W>À;'<b†ÝÕ?õ" pãÂÞ@±±Bؗ±@(‰‰V*"¿á‹³¾¥¿æ]'O7¿æ,‡JÀ J¿íÔo6"nAGNfsrqPMN J2331-2148?ïëWa8?^%³úB?d¨ïžíÇ)?^%³úK?ïôfîÀ=?cõ
g²™è?W3Ô""ì?cõ
g²™à?Ñ%.?šLÕ^ÁÁ?§Vòí­?šLÕ^ÁÂ?ïá0gÈ?jšè†•NÄ?nÏ÷˜þ8+?jšè†•NÄ3FGL J2334.1+0732@VôªŸæºµÀIM]߯' À9P>±·!À;œ‰çÒ¿¿K\¹ƒ2¿@*^%$QÄ@	À¿£C'¿å"«ÂªÎº¿èRk);/¿ëŠwV	L¿°qÀ•9–,AGNfsrqTXS 2331+073?ïüYÃZ??ËdkøÇ??í1å/ا??ËdkøÆ?ïñ®¶~'?d¶Sp.E?\£Ä"Ý}?d¶Sp.??ï°£w«%¹?½ÂÁû"?ƒ×"6'ª?½ÂÁû"?ïí&³V†?`²×´®?bÙL©yñý?`²×´§3FGL J2334.8+1432@X$՟Ú%{ÀF0•ÿ±%§À8èºÅcLÀ;<
MzÝ?ó
…örc@CÒÏÆ&j?þ
j¬¾d?äh—ë»ò¬¿Üƒm
¢ùÈ¿Û»ì,
þ¿àÈT˜ÉAGNbllNVSS J233453+143214?ïÿ,|F?ÅoV¡F?¿ºpw$Ð?ÅoV¡×?ïï¦;'[u?h~À•Ky(?`YÄؤŠ×?h~À•Ky-?îÁ"ë?š˜þç¤NF?£æ±a[?š˜þç¤NC?ïi™ºÌ?ƒ)%)&/?'ÌÜ(¾f}?ƒ)%)&/3FGL J2335.1-0133@U
>?Ö¯¥ÀMGy`>.9À9çÜÓ«
_À;–a(	4?äÔºŠˆ@)\šµ£@°Jߢ<€¿á|8xóÌ¿çlmiÃp¶¿åd*eÈö¿îáõrª¹ÊAGNfsrqPKS 2332-017?ïཊŽ‹?råÕ=t6Ô?oBuqúuC?råÕ=t6Ö?ïϗX¬³¨?€¯²c•?x4S©¦,®?€¯²c• ?î×Dp$ô(?–2C£å?¢‹¸ý°½n?–2C£å?í@wB›—?¡¹i#ŽOå?·ÕüEë#??¡¹i#ŽOå3FGL J2336.5+2356@Ym¢£Y6ÀAê.Íû¡À:SefŒ&À;àø‰éù-¿Ôl£÷ì`;@
"yöf#K@ã_`bÁ¿éD~Lêœõ¿ãKä;m-D¿Ü4H‰()·¿Ô/X×*ÁAGNbcuB2 2334+23?ïÿÐLíž?¹ ¤§?öbL)Q?¹ ¤§®?ïêã*´?n·_ß+åQ?eÕúKï¿?n·_ß+åR?ï¹óàu†?3Ér‰§
?ƒ‡âž]?3Ér‰§?ïî?Ý0ur?Uõ_°Ltƒ?aÀ"ϊ¡?Uõ_°Lt'3FGL J2336.5-7620@sIÈ MÀCú‹ Z›À9Ü-$%y6À;ΞÚK:'ÀßU®dÎ@é¥J§Ä@¤2`Ov
¿áre¼â
¿åÕï°Hÿñ¿å
1÷Ž¿Ú‰N³A`sAGNbcuPMN J2336-7620?ïöYx+ݵ?Wk¬FÑ?SM¨D—?Wk¬FÊ?ïóF8\Ñ5?d6[7Ãx?YsF]–k?d6[7Ãx?ïåîq¬?—j]ä£?ã\b1Ê~?—j]ä¡?ïÿäC°T>ô"8O93>ë¼O«äêG>ô"8O7
3FGL J2336.5-4116@u˜`@|ÇÒÀQG8à^*À95±/¸TpÀ;¬r9€
?óÙ—ïun@Ô÷!'@ê?Ðz¿Ü…¹}(¿á0ýg¹œ¿égÄ^á"6¿ä©ÀkžVAGNfsrqPKS 2333-415?ïõjàŸoò?Y}sÜ <?U*>Á I?Y}sÜ 2?ïôÕ0…
™?dÀÍn­–?VUžõäÍï?dÀÍn­—?í
ÿlû5Y?¥9øo´V>?·˜&U>?¥9øo´V??ïîÙ4Ž˜À?a«Í~ns?a&Ëqg>—?a«Í~nw3FGL J2338.1-0229@Uï¤hÀMâ'àÙìÀ8µçïhHÀ;n\Âxµô?à¥ß‰N.@sôI"qâ@÷®XëT¿ãæ!¦² •¿æÙ{ªD¿é"~‡øB¿äíëÅ­ÁAGNfsrqPKS 2335-027?ïý–D?3uÁ'-?3M؃ãW?3uÁ'K?ïó
Ñnþ+?d¦¡êøs?Yä]"«á?d¦¡êøt?ï€IÆ,q#?…™²Cª.?íŽtã·h?…™²Cª)?ïÚá4K×?hž‹7öËô?rþeÚ?hž‹7öË÷3FGL J2338.7-7401@sYPà"'ÀE%àdYFÀ9ʝ}SèµÀ;¦¶Iӈ©À@2¯´ì@Mlr¹±?þ4¢ÿžÜ$¿åÛá"ÒVò¿ãkܬ¿â¿Ê[ý!(n´¿ß˜Ëe;˜AGNbcu1RXS J233919.8-740439?ïÿÚDD6>î/{œÍå´>òÝÝä÷w>î/{œÍç(?ïõ˜OÞÈ?bP¸¸êË8?TÏÙ`Bmê?bP¸¸êË7?ïí§WNñê?o	M¡ƒŸ|?bX¨± ?o	M¡ƒŸa?ïÿÿÿðÁì=û˜þª×=Þ|&BXè%=û˜þ-ã3FGL J2339.0+2122@YPyámmÂÀC5ëß·‹À9ãIŠÀ;Àaâs'¿œô
Oûp@ρó_³š@nԀu¿ååª	ºz ¿âÑOS'ç"¿áАDõí¿ØswšÚûþAGNbllRX J2338.8+2124?ïüó''f?>/õ?8gnÃìΰ?>0)?ï䁙sç?uNabÙ?k~f~Œr?uNabÛ?ïœS²å»?…ýd"hw?ˆÿ«Fö?…ýd"ht?ïe:n¹B?"ÏL ä?"X²<(×Á?"ÏL ä3FGL J2339.6-0533@TUGÀ'áÀO<OøÃÌÀ8:[Ê+1ÝÀ;MQN§-@M¹2;;•@
‡ûÐñI¯@=I#àYò¿Øú"¯-¿ÖßóÙ^´¿áÇívÝÏK¿ìm¯nJ¾ôPSRPSRPSR J2339-0533?k2ž1[h?e´}b+"
?ïäÍaÎá¥?e´}b+"
?œƸ¿¯-?·äÎÓZ?ïiÊ:‡?·äÎÓZ?¯³:XðÀr?°~"LØÀ½?îÌZpóø?°~"LØÀ½?jWB¯Ã?cÞËþZ$á?ïåú¨½P>?cÞËþZ$á3FGL J2340.7+8016@]öaՈ@1Ó8€z
ãÀ8Kê¸pvÀ;$'ÅA¾?ìhSbÊòÏ@Q\ÿ_q*?þ¦½žÜy"¿É
BÖ
Û¿àŸ@ŸNÜ©¿Ù-ûȇ»¿àPºAGNbll1RXS J234051.4+801513?ïqNÙt:˜?Žwρ$å?'Ö$Ñx¬õ?Žwρ$æ?ìj"‰ Š?ÀË+Íöì?¿œ«[²û´?ÀË+Íöì?îA¼×Ü?žÅ$&ëT?«ä2Žß¢B?žÅ$&ëS?å¼ÜâÏ?¶®û¾ë?ÕȇF:c?¶®û¾ëŽ3FGL J2343.6+1551@YŸ'xÀEü_ !¸À:@µ¥8À;Ô+ç—r?éÿ»ä¬@´êÓ@Q¥ÿÙi"¿ä¶›Þuõ-¿ìårÐ×ôH¿àKcEŸœh¿åm{ 1ίAGNfsrqMG1 J234342+1542?ïÿ@¶žõu?Jl©l˖?é,!Qp?Jl©lËø?ïä{É`?v"}\ÞИ?k"6ôê  ?v"}\ÞЖ?ï/?Ó]s?"Ï?1}:?š"Qž?"Ï?1};?îGrZÅ¢U?ž`Ý@m•è?«ˆÚS¥ÚÍ?ž`Ý@m•è3FGL J2343.7+3437@ZÝþD5À:2Þ@'—GÀ:Iá`ÈWÀ;¼—•³[¿Öà"·Â@"†w}åß?üþ –
¿ïÿñ;äT?ïþ ûh%¿Ìi•Zo¸¿Ò·½áÍdøAGNbll1RXS J234332.5+343957?ïÿ-Zš\t?4ø¡–°?T¬´q"¨?4ø¡–±,?ïãCÛÆi?vàÊ&lʂ?l¼$è9—?vàÊ&lʄ?ïÕyd{¡L?s1ÒRP´?uCMÂ/Yž?s1ÒRP¨?ïó<×&Î?WGã®à›±?Y‡ÎQ²a"?WGã®à›µ3FGL J2344.4+0549@W'?ïXÀJ¢‹ Z›À:5¾ aŸÀ;·"ÌÐþ‹?âqš¾ÿüò@"ÕÁ=!Ÿ@‹‹À"§¿ã3Ál;¿®f@q<â¿âÿñÊ)¦º¿ïôV©"ôAGNbcu1RXS J234354.4+054713?ì'½'Ç…ý?¿3bÐf%?¾ÂiÃÐ?¿3bÐf%?äs3cÿµ?ÒKÔcÐ~?×ř8–?ÒKÔcÐ?ç@-\wÓ?¹iú…3S?Ñ¥Gþ[?¹iú…3S?áQvÉ6Ùh?½ÃRÙÔ?Ý]m'M1?½ÃRÙÔ3FGL J2345.2-1554@Plžà*w£ÀQ¿_ã•fÀ7>/GìÀ:ŽÞ¢¸&?ýdþ¿¹@ü½å©<¥?þ¹Rý(	^¿Ü±—¾ß5¿âFA¹¾J¿áº™ˆ@›¿æ¾ä½ëoAGNFSRQPMN J2345-1555?ï÷
o܄?Sù£€Û§_?Qå!ÔF÷ë?Sù£€Û§T?ïö®50?d°p¢&`?Só¢B?d°p¢&Y?í«µ¤R¬Â?£¢ø(?²¢RÝj™ø?£¢ø(	?ïÿÎàsXÖ?1´Æƒ>øÆS•r?1´Æ03FGL J2346.7+0705@Xß֔ÍÀJ/&à>™™À9*NRsj[À;1dÂ!x ¿ðò㯽Gt@ì±Ííß?üu§ALü]?ï]cdÿ¿ææ»"!àG¿Á÷=ëTÚ¿ØKÈ·AGNbcuTXS 2344+068?ïÿDnÿrð?OÀ%ø?r ¢á?OÀ%ä?ïóŸ@´Aß?d8¼‡f?XÁ~—|=»?d8¼‡f?ïœAàz«È?†gzvoۂ?ˆï‡áU
ß?†gzvoۇ?ïÿH?µE?#ˆpªzÍ?þx	WmÈ?#ˆpªz¹3FGL J2347.0+5142@\8åÏxyÀ#Îã¿ØrÀ87¢ò(§À:éß÷KüX¿ñîéµ:ßÐ@u'Ý7©?ü…2ªÍ¿ØGÏQâJã¿Ù	žkÝÁ¿ÝëØM*øt¿×|ÞÀó®AAGNbll1ES 2344+514?ïþOHÌ©?-Uçk?ñ?/;s5qÅ?-Uçk?c?ï'Èóz??žÂò­É,?‹MÿÃ!pÃ?žÂò­É-?ï»*ïWoê?'ßǂé?5D*$â?'ßǂé?ïÿšM×Óõ?Ð'"m1"?	lŠÉ`?Ð'"m1‹3FGL J2347.9+5436@\ož²gÇÀ"•¿ðExÀ:…gÖ¨î¡À;³0¨LÀ
­óõ"@ÏTБÓR?û»ê^Øþ^?ïÇôЙWw¿Ø$ë"/š¿éqF_®¿°ÿçÆ5¡AGNbcuNVSS J234753+543627?ï×*/Ÿ?xÐé¸Fƒ?tpðêè/ð?xÐé¸Fƒ?ßEo?¡Ù@í™]¼?Œøˆ.¤?¡Ù@í™]»?ítáÛe"Þ?¤ußiÑà?´Xñ$ÓY?¤ußiÑá?ïÿÿXß>°˜K> >"äÜ¡È>°˜KkŠ3FGL J2348.0-1630@Pe ÕúÀQøM@$³>À8@¨E.À;ýFèÞ?éûß+k‹@g
[@ŸmŠNοÖò"†ì)¿åG@ÿÞ*}рÕl¿æ—ÊšvAGNfsrqPKS 2345-16?ïÿ;u[ãÝ?du› ?'Tƒ"V|?du›è?ïõ'h¢Ÿ0?bÇOlèæ?TÛ.ºÁž!?bÇOlèê?ïKãÇ÷ÎR?_îfÆS•?–ƒ‡5¯?_îfÆS'?ïýY.î›ï?5ýüÒø²?56ˆ‹ "4?5ýüÒøÇ3FGL J2348.4-5100@tTŒ_¿ƒ8ÀO¦¿Â"OÀ:AÖ²ÿœ-À;ôäq.A?æxނE®Ð@|+Nbc¢@r?³Ê¿â˜ .wüU¿àØÉEiþ¿è&•GœÄ¿ïÿYsÜ1AGNbcuSUMSS J234852-510311?îêÚcÄK?¥ä!õÒ&‰?¡RYγ»W?¥ä!õÒ&‰?îøœµoÁI?©ÓηVþÇ? v4©ë€?©ÓηVþÇ?êª+C߂?°Œ@Êc?ÅWçRðú?°Œ@Êd?éLÒÈúì?±±ã_ZŸì?ˊ̴ÜM?±±ã_ZŸì3FGL J2350.4-3004@0ð›_lw"ÀS-ŸàÛxÀ9åÀ]RÁnÀ;ÂáåbÅÈ¿ìR@ƒl @ûÓ
ÔoX@¤ã@Ì¿çK˜³{Ô¿Ú·Éφ)i¿åÀ«°ÍÌ¿ÔÃUqÃß
AGNbllNVSS J235034-300603?ïü)»«r??ôÀùœ4?>²"£ôlª??ôÀùœ!?ïõBT>š?dV•ðùT?U{W'˳?dV•ðùX?ïˆdêW˜
?ˆ+ÊYÎð?æÅjý7?ˆ+ÊYÎð?ïþ§jΡ ?#Ëâ^Û?%‰Sî(?#Ëâ^Û¼3FGL J2352.0+1752@Y⮁ˆ*ÜÀE_H *AóÀ9èéuyÿ À;½ŽK‡½Ï?ÕUÌËJ@Á@ —ºœH¡@ô_¸Í<¿ë
õ‰Y…'¿³íÁ±]'¿Ý:O®áK׿çóijMËAGNbllCLASS J2352+1749?ïûYŒlK?GGg¥@®‹?B™Ï¦NÒ¼?GGg¥@®—?ï¿åã8ŠÅ?ˆ^j4ý"?€‡1ÝNá?ˆ^j4ý"?ïØ‰ï¦?ƒéM¥Ì?ˆ‰Ý¸¢?ƒéM¥Ë?^çå?"œ]¿''L?¦eº¯?"œ]¿''L3FGL J2353.3-4805@tw7À*ýÛÀP‹Ã¿ÝÑÀ:¯pÂ	û,À<
K³\¹?êgZ v±Ò@
ÕÇèa}É@x x™¿ì#ÞùÂq?ÝV'®àõñ¿Øhæ62õ~¿åÃ{GýxAGNbcuSUMSS J235310-480558?ïéå]d%ç?l[sòBõ?f¢›Új?l[sòBó?íQ¸$·'Ó?»¨š$6]?µr>ÚFÁg?»¨š$6]?îÀöÐÁ.ð?˜Ë¢GU?£ð'óí?˜Ë¢GV?ãCf8§3?¿T"ëŸ.:?Ùy3Ž°Åš?¿T"ëŸ.:3FGL J2353.6-3037@,*"øÀS8[ÿÛÀ9öøŠ/À;½Ÿ_¬8À
ågù8'@=L|ÛGå@Bm€ac?îþ>Ôüò¿åŽ-'*'N¿á4òX«¿ë@–®Ù¿AGNbllPKS 2351-309?ïü€\YɅ?JýÎå/I!?;ý1³Ýv?JýÎå/I?ïõ'†ŒW?cA_'UO?Ué°òçP+?cA_'UO?í¡çÐ9ô?£ÓìÏ
$·?²ðÁf0Z?£ÓìÏ
$¶?ïÿÙÒ3zb>ý;"^Å>óæBÍû>ý;"^(3FGL J2353.7-3911@u'ÒÀa"ÀR>"ßöu=À:š—Ëc@AÀ<Õ,ß@¿î¹Ò@Ö@ƒÊ${à@?[?kд¿çxS¨'Ï¿ÛQ´}¡¿à'-Èä׿ïÿZãÁAGNbcuNVSS J235342-391442?î¾'±û?²žUÔò?¤"ç/ W?²žUÔò?ïê¼CÝu?n`W…"Œ€?eCè¼"‹™?n`W…"Œ…?豏>YJ­?¾~i#_ÁR?Í9ÚÕJ?¾~i#_ÁQ?ïïðÜd°é?`³‹*ˆåñ?`#›O§?`³‹*ˆåõ3FGL J2354.1+4605@\+'ÿÀ/EšÀá@À9øÈHٍ¥À;Ñ*èáÖI?êÏ	\8ÿÀ@‡Á‰LÅV@Õ?qZ
¿ÞÆüE¥¿ä%~‹•¿îíi­÷'¿ïÿŒ"ÅÁ¸AGNfsrq4C +45.51?êµiåùIê?ÂÐûdԐ?Å*XhØY?ÂÐûdԐ?ÚjˆÿFúÖ?Ñ-Ê¥ÃÖ?âÊ»€\'"?Ñ-Ê¥ÃÖ?躦"	?¶vÇýšal?ÏágѯÞ?¶vÇýšam?ֈ‡£|¦?º` ÀÓK?仼.A¬ñ?º` ÀÓK3FGL J2355.5+8154@^7†6`å@3@à†7½À9撚Ϡ½À;ÊÛø¹º¡?Ú}'õ2@
áö#l@óðX•m¿épҌÄù¿çä{Óh¥ä¿èëh0"•¿éÃ剠ìäAGNfsrqS5 2353+81?ø#«Ù?ge¬¨4ô?‹A÷	B?ge¬¨4ó?íq(o]5?¹êå{û?´v¼…FY?¹êå{û?î9>À?œ~€Œ©Is?¬lÿŽ¨?œ~€Œ©Iq?å`ÿ"q[?¹vba)‹?Õ>ÙùI?¹vba)‹3FGL J2356.0+4037@[íÿ`Ï‰À5ÏÃøÀ9ávÐ@õ"À;ˆô›GõÚ»…Q¹@6û{6D?û+¿K"ä¿Õ¨ ,g´g¿ëvàêfÔ?ÑT'¹ó£ž¿×³δÀAGNbllNVSS J235612+403648?ïü,ܕ?EZÇiJ¬I?>™Sb¾?EZÇiJ¬>?ïä¤`¶â
?tÙ_q,}?k[ŸIóÔ?tÙ_q,}?契؃p'?ƒjŠ¢µ[?†Ý‰ß#ö?ƒjŠ¢µ[?ïÿݬ=Ò?Ÿn¦Ýß+>ñ)á1"B?Ÿn¦Ýޛ3FGL J2357.3-0150@Wb‰ۂrÀNËä€G¸üÀ:h_¿ƒ8.À;çCHT,¨¿»ù´PBýD@³±"
‰F@üªß'!U¿©J·'Ú¼¿èÀ/³ªoˆ¿Ö¯ƒÓV @¿ãk<P,,AGNbllPKS 2354-021?ïþŒU•ë'?.6#Ɯ¿í?':¦¡Gõx?.6#ƜÀ(?ïðéçim}?gˆ4¬JZ?^,1-%N?gˆ4¬J_?ï¦ì-Y#¨?€ðÇ~Ò^Ð?†Dô©·H?€ðÇ~Ò^Ë?ïºÞ0-ã?r›ˆ‹LC?`sô‡	?r›ˆ‹LE3FGL J2357.4-1716@Q¯3+¦ÀR†–ÿöÅÅÀ:~I±ú¹À;¢I
5
(¿ðz)˜Õ¤@I—ö×7_?ü×›£¿åàQ*¸e¿Ø'-˜‹ôã¿Ø,ßÌT¿Õé†lý?˜AGNbllRBS 2066?ïþŠÍåâ|?Ue­öj€?'S!¡Ø5K?Ue­öj€?ïóá÷.x?ef!BAõ	?X=Ú£c?ef!BAõ?ïÒбRm:?q Fg3!?v—§VÉc{?q Fg3?ïþ½tê7?%©œ"ÁÊ?$(¸\",?%©œ"ÁÎ3FGL J2357.8-5310@tz WŽ\ÀO~`X/lÀ9*i;,ü¸À;{ªÙ\þ?ñÑv—áނ@g%%ÿ@¤Ï_ÏŠ¿Í@&€ó/¿èh®\Ê0e¿éÛ7¯Õ׿èõI¯»2àAGNfsrqPKS 2355-534?ïû}N\·?B6%ÀzÍ?B
ƏÅ%b?B6%Àzß?ïðr
(Í?m…bÙá8b?_ãå®dü?m…bÙá8a?ìíy.T?¥×h)í?¸"3–t?¥×h)í?ïs£Œ"~?‡\pÀb?'‹Ž}›°a?‡\pÀb3FGL J2358.0-4552@tŽ§Ÿì™òÀQàÀ48À:
ÐW›ÈÀ;ñy¥Œ¿÷?ñ²ŠV@3¼ðáª@ïÕ`EK¿æîô´N¬¿ê8IÈuû¿äÎíöŠ'È¿µ"§?۞]AGNfsrqPKS 2355-461?ïÿ®£"×?	"N4®?W<^Ê"?	"N47?ïõêõœþ?c!ʒŸ?T*ÇÔg?c!ʒŸ?ïÜ`p‹`j?r•!Õ2s'?qÏǺOË?r•!Õ2s"?ïÿì×WÒ>åæõK?êi>ã(¨ð/Y˜>åæõK?ê 3FGL J2358.2-1022@Tæ@.Ä9ÀQDy î?À9ÿ`µL}‡À;ÛQk,žÄ?òYôèõ¢@é÷7"{¥@^ŀ'W³¿åãC;"ÿÒ¿ì7ä7ÍvÁ¿ï´xAk?ç€`'çαAGNfsrqPKS 2355-106?ïûV§m(T?HðLӂ?B¥bK^¹8?HðLӂ?ïõ«.ø·6?_šÛ $¯w?T©¢'"Î?_šÛ $¯n?íæ%÷?¢-]øbÕ4?°Î׸C—n?¢-]øbÕ5?ïd"<à"?£…ÃØ@Í.?"~
xcí'?£…ÃØ@Í.3FGL J2358.9+3926@\"aùðÀ6NÚ_\†êÀ:DýòÿfÀ;¯&2™°@À‰£µQ[@½v›<ÜÕ@ªóŸõST¿âDè´¬<¿àÖÙI»h¿ïp J3'
?ì–Î( ÞAGNfsrqB2 2356+39?ïõÔÁ8ê?[¯÷6?TV}ێ-Ë?[¯÷6?ïå'CP™È?v؜Œÿeñ?jn¼¯f8?v؜Œÿeð?îқzý4?–P! ?¢ÖH^ ,È?–P! ?ïÿÿ¶'zŠ>'‡«O)™V>'_a]å^>'‡«O)Jÿ3FGL J2359.3-3038@)iÄupÅÀS"x $ÎÀ9½¹Ì?TÀ;¶°ê7.¿àêìX@
³¿e=W@,7žÞ¿ç1Ro°ßS¿ÞlŸÖI£7¿áœ¿^­½ñ¿Øê|"îËAGNbllH 2356-309?ïýˆ«Áû<?0cõÈw_k?3º¡ð&$I?0cõÈw_™?ïóç'/€Â?c¤1½zß?X1± þ{Œ?c¤1½zä?ï£GŠm"*?išü…'K?‡.dšõw?išü…'G?ïéûXK
?`%¦A" ?f§p´ö´?`%¦A"3FGL J2359.5-2052@Lù>À//˜ÀS'*ŸæºµÀ:Nè},{‰À;ë?Íui9ÀLEÓÉÁ@»ž6aeö@$6ßæ+¿èûAîs ð¿Þ",æ½å¿áZ˜U²ö¿¤­ca4ŠAGNbllTXS 2356-210?ïþ¾:jDx?'¦ÑÊ?$Y[¸~Ç?'¦ÑÊ	?ïöU¤e"€?`¥kÄÈ?ST·4Ù&?`¥kÄÁ?ï°îGyT?}þÆ[°õ~?ƒÄn!›êë?}þÆ[°õ?ïÿäl¨»M>ïYæ¤OÒ>ë"WD³
>ïYæ¤K(3FGL J0000.1+6545@]lh‡¨ÖM@9Aâù^üÀ9ðÇô À:æåèðð?óÇî@
©ÛÖU@I£@Œb$¿ÜTX
ÇÉ¿æRGÀ*tj¿í$[ÒK+¿ÕÕ¤l†fUNASNonenone?ÌìÂÙÃæþ?ÌÓf‡Çóª?èÄÏIA?ÌÓf‡Çóª?åþCñÒûG?Ö/\=5ý?ÔxZ	s?Ö/\=5ý?ጜ?¹œDç»B¾?ÜçÇÄÇÅð?¹œDç»B¾?БQdhÖ×?Â÷°æÿ†c?ç·WM˔–?Â÷°æÿ†c3FGL J0000.2-3738@u–'}keªÀR¼—žÖÜÀ:ÀঞdÚÀ<åS¬O?ÙÌd3ӎ@lþ.ϐ?ýÞ"?pq?Ã}¸X‡¼´?£ß!W tֿԐÞÎX¿ä½÷n®UáUNASNonenone?ïð‹ÐŸÞ¥?d®\ÔúLå?^è^ÀB·^?d®\ÔúLå?ïí"LLP?kj% ä'?bl³³ã±Z?kj% ä)?ï9Ähf?'+"àÍO·?˜Çrüs<ƒ?'+"àÍO·?C%m>?~PlQRk?œ¯6¤°g?~PlQRl3FGL J0001.6+3535@[êU!š"{À:0AÿŽÁÀ:iTz«—ÉÀ;Ý+€À…¿þ³LØç@ÒèDÍdw@ÍÞ?eñv¿í"O'…€¿×òp'@ƒö¿äSÿv¿Òw:/aÿUNASNonenone?ïö0(²?XÖÎ` !J?SŸé®›Ñ?XÖÎ` !E?ïçچ›H7?r°_v¬¬³?h%yd·ÈÊ?r°_v¬¬²?îìø£©ö"?–fUï˜è?¡0uÅ`–Ë?–fUï˜é?ïÿOaqa¬?؈v«BÚ?ÑÓÊ}È?؈v«Bë3FGL J0002.0-6722@sb9-Œ*ÀH‡ê=ö۔À:n»ØˆÂ²À;çŽ
^v?ÔQn:Mâ@¦€®ç	?ÿ#?B‹?·m¸\Nj¿àºj­{^¿Û"Ï2r¿ßÞqƒ±êUNASNonenone?ïï΂O ?gnl9=õ?`1}°ßð-?gnl9=ö?ïì…ݪ1?l,Їî{=?cz"Uþω?l,Їî{D?ï_©Ê»wÉ?-¯¢'¼â?"
ƨ'Ë?-¯¢'¼à?ïw:qb՝?€Å\Iïó?'±Ó¥Lm?€Å\Iïó3FGL J0003.4+3100@[½³R¨CÀ>¾¾zúr"À:v,­5À;à/Q&cA?ÑGˆ>Rv@
6v5ƒ@nB@p…¿æȼ¦º¿ãVîÆ
ª˜¿ìžr"Šq¿ë÷[DŽ—UNASNonenone?èìõJD›s?Ær­).½s?ÌL*Öí'5?Ær­).½s?ç1X*ca?ДÞBƒ¬`?ѝO«9Å<?ДÞBƒ¬`?ì¹Îþ.‡?¤ìïí¦Þï?º1ˆÛÍ?¤ìïí¦Þð?áôԁ,Y?¿µWK'Ï?ÜVý§ËN?¿µWK'Ï3FGL J0003.5+5721@]Š	ÞÀ¥yÞonÀ9ó"#]ÓÀ;…KQ7*9?ã,%2£v@€ÎۚÅê@vç?¿³Š?ïóšÇ'X¿ääëÿd.¿åÌ3Õoˆ¤¿â¾j}£ÊUNASNonenone?î¸N¹U¶?­iäz¾ô?¤~»j¤˜?­iäz¾ô?â½åogKž?Ön~Æ¿_?ڄ5!1hÃ?Ön~Æ¿_?ëáSÇî?µšzÓ¬I?ôz³ÄàI?µšzÓ¬I?àN£4l¶?Âdu*7¼×?ßb¹—&'å?Âdu*7¼×3FGL J0004.2+6757@] •þÚf@ùÛ"Ðå`À9&ÀÀ:×t4…BÊ?õÓ.»ª:§@fyHì-@ù…±;!¿—è–¤>/³¿éì¶¥K²¿ålÙ¿pæ¿ëN§.œdiUNASNonenone?ª–®o¶Ü?²uI%…?îVže'?²uI%†?҈×IJHË?ÒuÞôí?滔[Zۛ?ÒuÞôí?ÑÎDã]E²?¶/¢3®Î?çݎQ]'?¶/¢3®Í?°tf²¶5?VîTôÎó?íñs)©<Y?VîTôÎó3FGL J0004.2+0843@Yæ^NÜÀJ.ý›¡²À:‰Ù\'HCÀ;Ü=TeF¿ÎJ¬)FÔ@ƒš›ø@gN``=¿è)þ_R16¿Þ'&ˆªÞæ?CC瘿ëÜC·(ºxUNASNonenone?ï3å˜âŒ?™ª;æp¹?Œ3™Ç\ú?™ª;æp¹?ïççtS7æ?r	‹¯Ò@ž?h‹¬ÈÁ?r	‹¯Ò@Ÿ?ìåŒÁ½?²BÅc3{Œ?¿€×S™ò?²BÅc3{Œ?ïß,KÝÕ?u&î'U&<?piûÚ^?u&î'U&<3FGL J0006.2+0135@Y¡ß¹8›ÀM¥ÿ¼ä!}À:gÇÐ䉂À;åÅÌ'‹_¿üuB¿Ã$@§¡ïÿW@~Å ]®¿ãÙCӔg¿â>$A‡¿ä§³ª*Ð'¿ÙJµïˆUNASNonenone?ïüàñrf‡?9{Fu%?8øtlËĘ?9{Fu?ïôðˆÒÄ?b¹›£Ì?Vî[îx5?b¹›£Ì?ïxJVŸ%'?ˆÅ.ÿǀ?öµ,[?ˆÅ.ÿÇ?ïÿ¾\b¢?t孝-ù?hýçW±Á?t孝-Ú3FGL J0006.6+4618@\ºÚQÎÀ/»µà÷üüÀ:4š"U•^À;µ/ê©¿²¡¿ï‹ìò@èé­@VŒ?"鬿ëªü ¶*¿çùÖŒ
˜¿æ÷/Jàè?ªƒÉ<Ž@UNASNonenone?ïì'lsÇ?hq3Q[›U?cØ铌9?hq3Q[›U?ïÍ­BGÕÓ?ŠZþÈ¡?y)^ܬ?ŠZþÈ¡?ïOt~צ?Žµ \_¹?–p=%F?Žµ \_¶?ïïûC-?[¯g±ó¶8?`¼ûÒÿK?[¯g±ó¶73FGL J0007.4+1742@[<ÝÖàLÀEô™÷LÀ:kå˜u­+À;âƉ¼­¿ÌûÛqïö6@ºS«x¿.@~á`'¡°¿ãøÏE^?¿äl¡¡¥¿åx¨åx&¿Ý@—UUNASNonenone?ïùsYvü?Q#/5Ú?J3þš$°?Q#/5Ü?ïð;L~$#?h8¿éy
?_‰g·¸¡?h8¿éy?ï<üŜ%Ó?¥L€è–?˜`gL{E ?¥L€è"?ïÙ[iæéf?g'õBåù?sRK‹M'?g'õBåõ3FGL J0007.9+4006@\~‰ô
(xÀ6Ø@žUÁÀ:[	Pá™ãÀ;Ï®KØE§¿•Yl‹w¥@Xö§¼@4p yr2¿ÎBœƒj€¿é$íú]Ãn¿Ýn‹ðò›¿âÝ«{]2OUNASNonenone?ïùÝí>Ð??Q›‹PÞ?HˆK¿Û?Q›‹PÞ?ïԕîVÊN?'À–3Ól?uµԚØö?'À–3Ój?ï-f9º*ö?"+:B´Ál?šS8Ⱥ¡2?"+:B´Án?ïÂß5Mº&?oD³'ã(Q?~eY"ìÇ?oD³'ã(M3FGL J0008.3+1456@ZënÀY!ÀGT<}^ÐpÀ:W´üÀ;Ï÷1$e:?ÜÉr¢éO@PM7–DP@(	_Ð=¿ß¬Ýƒ€Ü¿áqK²0n¿åT†e<ù8¿å£Y
ÄeUNASNonenone?îAh~:ñ?°¹&·xœ<?«éxPîþ?°¹&·xœ<?îýaÁÐ!?©Å²àú';? .éãâýé?©Å²àú';?믎ÔH?³õÓX(ºŽ?ÁAÇįâã?³õÓX(º?繤 N?³Ÿåc(	?Ѝð·ÿ¿d?³Ÿåc(	3FGL J0010.5-1425@UbMÒñªÀR‡&k¤"ÉÀ:"¢ïƒ°úÀ;þŸ¹™ê?ðÃ?ó`	€@#v4åç@w_»ýG?ï÷"ÁÄO¿åä6j—šÞ¿èŠ(‰¥Ên¿ïÿ†S>ÁUNASNonenone?ïžv-bËÕ?ž£ªÛm®?ˆbt§M
¨?ž£ªÛm¯?íJϞŸ?¿«ŒN"?µ©ƒ7…?¿«ŒN"?å\±u?·(×ÛUÞ?ÔýFÏß?·(×ÛUÞ?áG:"-?Àéùlbð?ÝqËË»¤?Àéùlbð3FGL J0014.3-0455@XåÄØì–ÀP†"&þrÀ9ÁÉ@PR(À;råB˜I?¯ZP ²Z¹@÷ä÷»ãÆ@MŽÆ,¿ãVaHæ¿êx.ÉRU¿àhà1®y¿ça6+¾¨OUNASNonenone?ïÿ!<?÷!ÜÅQ=?·°ûøúË?÷!ÜÅQ+?ïñ½*Áu?f
@¸€°Ú?\…ª}÷?f
@¸€°Û?ïÅ<ÆÎ R?zë‰{T?}aœ˜ïÖÙ?zë‰{I?ﵤ8 ÎÚ?r#îbnˆ?'–ñ×ÌIe?r#îbn†3FGL J0016.5+1713@[ÉÐúX÷ÀFlÖÓõ¶À:n‹†±_‰À;ß-(W7?ê	UŽIPÎ@¾¨×Ð@D`Þ<¿âŒ]`â¿ä¸—G¿íDŽ $ô½¿Õ°æØÍ®UNASNonenone?ïà¿úr`?s]¥öt?o@ŸùÓ?s]¥öt?ïÜ>Aü£?Í"DLÃ?qàßð.V?Í"DLÃ?íºÊlL4:?¢šj"Õ¯?²)¬ž^1?¢šj"Õ®?ìS -}Ñ?³%þ©ë–w?½fþ"Ñy?³%þ©ë–w3FGL J0017.1+1445@[«úëÄ	ÀG¥‰›õ"lÀ:"ùdoÀ;Ô_rV_?ĬÌɔ*'@³0ÅŜ'?þ àÀt¤Ã?ïûÛµÔ¹¿Ú›j"ÍNA¿èÇú¼#\?¦´+]UNASNonenone?ïâ?ψ7?v‡R
âúÇ?mìÀ0wÈÇ?v‡R
âúÇ?ïí»¬†ÁE?mŒDPBn?bDSy>»Æ?mŒDPBl?ídBõ_Ó?©ç(X0þÍ?·\ÝèUh?©ç(X0þÍ?E="?ŒPƒóRX?~.°šì?ŒPƒóRX3FGL J0020.9+0323@[ªà"ÀMLæ¯ÌáÆÀ:Š£×
=qÀ;º™?׆d?Û±±=¥'@ù˳G@?ú=	þ±vZ¿ïöjÌ;?ïüÃ'I¿É§Õ"Öó¿Þx&ŸH|"UNASNonenone?ïÿ/̌n®?vbÆó?nr*1–?vbÇ7?ïðœq‰F?go/!fnõ?^Çäíuº?go/!fnó?ïÁ)xgÌ?}cD@x¶?kCÌý?}cD@x²?ïÌ ]#]%?ujã}¹Á?y¯ÑnQmN?ujã}¹Á'3FGL J0022.7+4651@]uõ׈²À/xpCßÀ:4Õh-À;ºÊá:B¿úŸ/¸ªUÿ@
"€`7£/@F/ßÁœ¿ë"Øz³ƒ¿â"ß½Y+.¿çŃþZl¿ïÿî¼zˆ÷UNASNonenone?ï"uZïb®?˜,†At?Žâ©D'Tf?˜,†At?ïXÿ!/%?®þ‹Ú0l?"ü`ځ?®þ‹Ú0l?ìZ°'"È?©ÖKîÃ_(?½*{ëa¿7?©ÖKîÃ_'?ïò"Kƒ–?`§ÄìêcC?[»iúø×F?`§ÄìêcG3FGL J0026.2-4812@s¥í»YÝÂÀQ°J¶¸À:[7 '½´À<
Õ«˜ ¿Ù-jôb	'@ŠBÅøG@ù1~'¿Ú/õ¾*¿ÝOõd}¿äï7+ª¿á{Æ!ü™UNASNonenone?ïàùö#»¼?€»ƒ(þ?o	ÜDC¥?€»ƒ(þ?ïó7ò§¤Û?d—íù"?Y°¶Iß?d—íù!?îHe%k}?¢m»õ/Í?«©­©H)?¢m»õ/Í?ïî?¼T°?WÁ›ÓZ?aÀCï«Oò?WÁ›ÓZ3FGL J0031.2-2320@Qà% …²ÀUŸS À:§H>]À<
àO`d?âêñ3ša@;7äs@ç`Kð?¬ûÕ¿ÜSÜÉ͜‰¿â—=x¨Õ™¿ïøô
Œ
HUNASNonenone?é¦ë="Vé?ÈMDF#r?ÉdS	²¤Z?ÈMDF#r?åVÛH¢{¬?ӎÒÆS?ÕRIn»§?ӎÒÆS?èe%-BY?¶ðgãç—ó?ÎkkJ÷š?¶ðgãç—õ?àìIóî?ÀWÊ74.?Þ'l#ïú?ÀWÊ74.3FGL J0031.6+0938@\¶ñ€
|ÀJtîõÀ:.´iÿxÀ;»²åšùì¿ßçQu
›@
ãtÈG@Aë>":¿á‰Ñ¤fÀî¿ì€|Má¿â
N×æ¿ÄÃ9TyBÑUNASNonenone?ïÿj'!Bå?ú•Ðù?»×£RÞ?ú•г?ïñ'\Ù}+?f•†»Žó?\ûFM¨ü?f•†»Žò?ïfæOü?cqp+ª?"<C6 m?cqp+§?ïß @¾tÜ?h©-Ë'?poߠőã?h©-Ë(3FGL J0032.3-5522@sI輜$ÀNÆ6!úü‹À98ҙ•gÜÀ;ÆNóƒû?ÔVÆÚ´/â@ñ=ÐE'@2YÀe¶=¿×†Pn¿åÀ_±krj¿åþ.æ꨿ãú¹˜xÃqUNASNonenone?ïÿMz'"?v8ž/?P­¯|ñ?v8žT?ïõv6£~?bR¤¤‹äB?U'¹ÍV?bR¤¤‹äB?ïaùØÆBZ?Ž@ª8G'í?"ÀÄç7´Ç?Ž@ª8G'ï?ïÿìÔLæG>äÌlÊ28>ã+³¹»r>äÌlÊ13FGL J0032.5+3912@]¼ãÿï9À7ƒIàâiÀ:L‡È¶½—À;ظÙÐÁN¿ØûÒ4{îÊ@|ž©£ÒØ@'â?û˜'¿í–W£]›¿ä®Ús~|Þ¿à¹ýЃn=¿àFÊڐŸUNASNonenone?ïÿ3ŽZ¨? ^Ðùì@?Ž4®®? ^Ðùìu?ïÐ:ÉùG#?ˆ®]ƒÖÝÉ?wâ›\n?ˆ®]ƒÖÝÇ?jlº"?…)'*C ©?Œ—edÑ_?…)'*C ¨?ïÍÚ I6?n}Øb\?yø/Ûdß?n}Øb[3FGL J0048.1-6343@rø‡~äâmÀJ²D¿L±‰À:G./¾3­À;þö ƒ-G?óeø¸
"'@šUéŸì@Þ Z¾h?ïú$ƒíàÄ¿Ü®x¨‹ò¿âÓ2þ§L¿ê‡'éô'UNASNonenone?Ú°lÑu`?Ð*L!Ò?â§É—}ÅP?Ð*L!Ò?ì£ÕN…èÐ?½Âr<C'?ºáU‹Ð¹?½Âr<C'?ÐPÈÓ"?¶ïâï0§?çכô–w¶?¶ïâï0§
?à ýÐ?¿ ã#r õ?ßñ¾Åþ_?¿ ã#r õ3FGL J0049.0+4224@^'Ó"wÀ4tÙù9üÀ:mã؂µÀ;Ò?R%f¿Þo£78a¬@""^žñÈ?ü>ñŸêìs?ãˆ)ºc"£¿çÏÅ^)½$¿Ë÷W<쉿ÒIûÒ·ëUNASNonenone?ïý ±–,ú?@0ÇÂϕ?2úsN˜73?@0ÇÂϜ?ïÇڒf"?"ÎÝd]`?|¶Ì¶wP?"ÎÝd]`?ïnޟ®?†x5waÔ?¤HX~P?†x5waÑ?ïô†6Ǘä?T¬[]WÊå?Vó'pÐ7Ë?T¬[]WÊë3FGL J0051.6+6445@^¼âCV–æ?þ3:ß¿À9†'•ùÀ;&±¥ÿÙj¿ÇùlŸÝÍÈ@MB¨ñü1@;ê€fí ¿âÃÔe>ëp¿â u¡<¿å®ò)伿ç:ӓÃõ@UNASNonenone?émWP"»?Èi1ï[æÊ?ÊJ¢½íâ?Èi1ï[æÊ?é¨k7†ä9?Ït|]S?É^S!äo?Ït|]S?ë®âãJy?®-ñ±®'$?ÁDtr×ê?®-ñ±®'$?î…—½æ€?žh¯—´×?§¯F"!—ý?žh¯—´×3FGL J0102.1+4458@_;6;%pÀ1ÛÇæ³þ À:‰–Ob=ãÀ;å¡ÔÑ~¿ðV+57ð1@
§òz†Xõ@í@Š´¤¿çíô¬²•¿ìÈÒÊÆ@?ʈJ´%®]¿é®þn–œËUNASNonenone?ïüYcŠl?@Á@ŸKl?=4レ¦?@Á@ŸKk?ïÏí½³æ?"ÓøKŠæ?x	}¡&Ï?"ÓøKŠç?ï`΁E{?•‹9'ñ?ž3æ/×PÃ?•‹9'ï?ïþŒƒfÈ?6!8øŠÓn?'>—É"?6!8øŠÓ3FGL J0102.1+0943@_Õ*¾ðk8ÀJ†«Oœ À9üÙ~‹÷À;¶Jt˜XQ¿çef#þë@
ÚŸƒéY@…*ÿ²þ¿ÓU3À™/3¿æ)"Á¿à<q—5Õê¿Ó14iØЀUNASNonenone?ïþoí?1:×¢SZi?/>™Q;ã?1:×¢SZ€?ïòÆGTpé?eQchªE?ZsqW*þ?eQchªF?ïþ²*#Ã?†vúª®ý?ŒSuwJ?†vúª®û?ïù ›ˆ²»?El,ã3k?K}'Ý5…?El,ã3d3FGL J0112.9-7506@rÑ.Hè§ÀDøûüe@ÌÀ:o5·qñµÀ;ùRÈ#ð À°§ø¬út@
m…6‹,n@`ŸõÔ-¿çÅùÛ	¿æZÅkY•H¿áªú_à˜å¿ÙúÛö,äÝUNASNonenone?ïÿœIY¾§?	#ZX=d¨?í©VEß?	#ZX=en?ïó®Áè¨Í?dÊ	7EÇ?X¢|.®f¤?dÊ	7EÇ?ï̤E¦>v?uNHï3ðl?y­Ý,àÅ?uNHï3ði?ïÿüñÝÁU>ɬêOlV>¸qõY‹ê>ɬêOl(3FGL J0114.8+1917@`P§æšÔÀE¯ž¾œˆÀ:•k/ùÂÏÀ;âCæߝŠ¿âlä{%vm@
1_C1ƒ@{] :¿ëḯéÅg¿Ï·zn¿ä)nDÅñ€¿â¿#ì:È UNASNonenone?ï÷áÐéëÅ?SÃFßæŽ?P<^,(w\?SÃFßæ•?ïí
«k?½?nãLoÓ?bòT"ÀB7?nãLoÔ?îÝÅFO?˜Ûa¨›?¢#«ž.K?˜Ûa¨œ?ï܌ý#÷Ë?g™'äË/?q¹nò?g™'äË-3FGL J0116.8+6913@_L³åu:?@ߑæFñVÀ9xÓ³pÛ4À;04	t?ä§ÉJaM"@eQ5|¹@ à_Ñ¢¿æ` ÇJ×À¿ì°Ê!:§
¿è‹êפ¿ïýôf]›ÖUNASNonenone?ïþ'M'?šÛ
/âyÓ?€-Ö[ç?šÛ
/âyÒ?ꚕ¸˜øÓ?˜–.%S?ŕ©œ´?˜–.%S?êæn'ê3?°ìÁ?ÄfGùôW3?°ìÁ?ãŽ{Ä^XÒ?¸«ÊO2Ñ?ØãwCN\?¸«ÊO2Ñ3FGL J0127.4+5433@`3:}ªÀËDå^³À9êÁþ<±aÀ;t»ÑÒÆ¿ä<™$˜'@·ºt°@B‹ÿÓ	}¿ç]Ñ`¥•¿äÔºLA¢¿í–úNÔé?Ç z^ò\UNASNonenone?c~CH?'<û¼÷™?ˆÑ§ o-þ?'<û¼÷š?ïCêIG¨;?§ÖJF"W?—'¶×
øŽ?§ÖJF"V?îK8X<à¹?›œfoÚ?«Lz|1ôr?›œfoÚ?ïê/¾ç&Ý?fE`´Êf?eÐAÙ"'?fE`´Êg3FGL J0127.5+5634@_û
å6PÀÏbùÊ[ÙÀ9†}™ˆÒ¢À;V¶7_Þ¿ñîJ 	¶@åtìf;@°ª_d"¿á>ûù`(µ¿ì•
5üó¿åPS«‰í:¿ÊÑPŸGƒUNASNonenone?ïç š-Hš?qk¡!CX?hßeÒ·eô?qk¡!CY?ïoÒCÖ@]?¤¬—Ó,Ù?'·…7ô^?¤¬—Ó,Ù?N?œ$>®ˆû?¦f~+%?œ$>®ˆú?ïþM\
þŽ?*%6Q8O?+*? ;?*%6Q8O$3FGL J0127.6+4851@`!¸'ú
À+(iƒQX¸À:ÞC핚À;¬RLÓî)¿üˆà¡bç@Ñy[á}3@•Û_⓳¿á¨Æ0o›¿æ«2œ›'Ô¿äH-û)Æ<¿è‡S@]¾UNASNonenone?ïýîh 8 ?5´û®ú#?0Œºþ;ú?5´û®ú?ïÖ^BV"?'Zt0˹?tÿPÞÔ¶?'Zt0˹?ï­ÓÖMˆ1?ƒ@vž>?"‹
ló¼?ƒ@vž??ïÿ‰ÊBR¤?£ê×1!?
okVÕá?£ê×1Œ˜3FGL J0132.1-5340@rÀˆPœÀO4MUhÇÀ:‰š8ûÊÀ<¨Å†‡n¿áEÉ_ÒE@k~K4†Å@Ž#"ÅÊ¿†Ÿ
[sz=¿æjÉÍhþò¿æƒþ8ø¿á}ØÚ"UNASNonenone?ïòc™mõ?b¯Ý¸?Zå8Í$°?b¯Ýº?ïïÃœ °?hÈB4z?`<æc_O§?hÈB4{?í× ƒp¾è?£Õi•e?±Fûäz¾?£Õi•e?ïÍ;<·®?q	3ºŽªØ?ybaþ¤)?q	3ºŽªØ3FGL J0133.2-4737@q¿'»/ìÀPü_oÒ À:/Ùâ_À<Ê~=ó¿üšg<z.Å@@âH_@¨è?Äæú¿çÇoE»©—¿æ¢Ißô¿ìä
‡Z°?¸K{Íð}UNASNonenone?ïûw_u–ò?M 2ø+ƒË?B"')¤;Ù?M 2ø+ƒ½?ïõg+¼É!?bUË˶²Ì?U1¨†m¾Z?bUË˶²Í?îøøæô?'þÙ£ŽÛ? ~ðq¾q?'þÙ£ŽÛ?ïÿ'+
òÄ?'áÍ0†?u=COJM?'áÍ0†+3FGL J0133.3+5930@`pyåŸ,Àg±j4À:
ˆß72œÀ;i)¾?kP¿áÞÜ°UÙâ@f
uú®@±?ÿÊP¿Î¹¸|*?¿è9@ÔB¿ÓÌ8+¯J¿êwÎkûCUNASNonenone?ïŽå$õC%?Ä•¢ˆUò?ŒF¶Â¯6ô?Ä•¢ˆUó?¦à¯‰?¶VcÚ?¦&¥'õh?¶VcÚ?ìñ$D]X_?¥Âpk»l?¸vÝÝ=?¥Âpk»m?ïÖBD®?sì•Ý°?tÞÝùø(É?sì•Ý°3FGL J0138.5-4612@q<w¯dÀQ0Ý)4­À:W'hr°!À;õo|ž¿â
Ô1£™«@
ŒŠâq¥@|äpùg¿Ó1{©Ñٿᇜ|
9¿áT¯baR¿â¹'£¹¶£UNASNonenone?ïñ¸ó–P6?eϾ(Ë`ï?\ŽÓ_"¤?eϾ(Ë`ñ?ïî¨ÙÿZ?m›]\uŒ7?aîW&¥˜?m›]\uŒ6?îÝé«(=Ž?˜Tãé
W!?¢!eM|'?˜Tãé
W"?ïף㔇e?mi'ÜÓop?t.5¼Lþ?mi'ÜÓop3FGL J0149.6+4846@`—*0U2aÀ)ûԌ´®ÉÀ:K8ãv\À;œ˜È¹AÖ¿‹#ÔÛX@šq¾3Vï@õ `]7é¿ê±®B•s<¿éªŸlRŸÆ¿×K4Õ'lß¿ãŠò¯+ôUNASNonenone	?ïþøXö$Å?"q`¤Àª? zp³¯7?"q`¤Àr?ïa Áph¢?¦R3ôR¤?"ËçÑòëÐ?¦R3ôR¥?¯ËÑ?ƒ`>iLÕ?ˆQÔ
¹?ƒ`>iLÔ?ï|—X¯Zð?Ã†§0gô?mê¢!?Ã†§0gô3FGL J0154.1+4642@`¿rSÍÝÀ-£Íi8À:DPXÝèÀ;¹—×øyú¿ñîW@َý@
Ð1Ü@j›`n)Ô¿çLܺß0¿â€w€ƒâ½¿ïÿËeªºå?ïýø£ë,3UNASNonenone?ïÛr@¦?z',"§?r|Fßÿ­?z',"©?ï×Vz¨Ž?ÙfÂu?tTðB«¸É?ÙfÂu?îUˆª©Ãù?›r	ϖ?ª§uUcÀn?›r	ϗ?ïÿ¾§ï?²ÛÉMÈÐ?V<hØ?²ÛÉMÈ×3FGL J0156.5-2423@i¿m	Ö¶ÀRÆÍÈuO7À:žr©jÇõÀ;äçW'Ž
?ÇÛ_¦r‰Ï@;-Ö'•?þ7>ÀZ#?à);Þ'"¿Û0š5ò¿â°¡$Ÿ¾ï¿ØdÖ°LUNASNonenone?ïøÈcˆü?U">B
D?LÞqÜ
À?U">B
D?ïòž•ÆÌ?eªÎ­O,?ZÂÔsÞi,?eªÎ­O,~?ïW¥:*?‹þkó̱ª?•‹NXº³?‹þkó̱ª?ï¹>N¨m?s÷C	@µ?¾ðlUäê?s÷C	@µ3FGL J0158.6+0102@cpcŠ	ÀLÁ¯ ê[SÀ:1únƇÀ;Å;"ë½S?Ö¨j²@P
;§Ëá@wÑ߆7è¿ç2rÓ~¿íëMƲV¿1š°.¬G¿Ò'¹'Õ§‰UNASNonenone?ïÿ²9د?óŒÕ÷Z?|ñ‰Ô,µ?óŒÕ÷Z?ïóœãqèû?d
móFöQ?XÆ9.	h?d
móFöP?﵁"<¨Ï?€¬öåž?'ŸžðÕÌ?€¬öåž?ï꥞γ?bd®bÂé?eZa1Læ‰?bd®bÂê3FGL J0200.3-4108@p`ì"h	ÕÀQ…=ÈK^À:o×½Á—À;됝T9¿åþi0O@Å2í<™?þüÀZxœ¿ï¤Ew¶ùY?êv–§Ì¸*¿ÞaË.žW¿ã𝫐ÖÁUNASNonenone?ïý¨*'¬?7Ù7be@?2¾«rŸ?7Ù7beN?ïîuÊø?nª ªÇ‰œ?aŠp5ù?nª ªÇ‰š?＀õo"?}ªâM!Çt?€ß½ä?}ªâM!Ço?ïîí	eå?a^ù!}Ê?aö÷šD?a^ù!}Ì3FGL J0203.6+1148@b°r\=îxÀG§>›A:À9̚`hödÀ;lQÕµ©›¿v¸ŠF|¨}@üçá¦#@·SàQäÏ¿å]Y¸`·®¿êÝÍç½g¿êÙ0\áyÏ?Лü,XEUNASNonenone?ïô¿³0t?_IO¢‡g?V€™ÇŸ0?_IO¢‡b?ïñiaÄ´?iÐ=7ô‹ó?]-ù<v˜¾?iÐ=7ô‹ð?î©l0´Eá?˜Wz¾;?¥i<ô»¡ì?˜Wz¾;?ï³êä&Ø`?ƒ×‹~ºÜ?ƒFöIçù?ƒ×‹~ºÝ3FGL J0211.0+1922@brVWûi˜ÀCÓ<ŽXÀ:%S'^²À;²V´A»Œ?ÀV
1tu@
µ4¢žûÙ@•€r+¿à`3$ª¿éN·ñH'%¿âoÛ
 ¿ïÿH¯
2ùUNASNonenone?ïûéNŒ)?Lølq‹#?@ZǽÏX×?Lølq‹,?î
i¹Öç?¶BÎt–þ°?¯.	db'œ?¶BÎt–þ°?íCVUËä?¥§")¦?µåMQ¡âß?¥§")§?ë>uA{È?²s\"ïäì?ò*úâ?²s\"ïäí3FGL J0216.0+0300@d
\|ؘ³ÀJÌ~bÜn+À:§.~˜ŒSÀ;äȁäq.¿êàB&"èÌ@
!Í°!›@2@·¿êVbÉ_J¿à(³éãQ¿Ø2|mӇ¿ã7µeó UNASNonenone?ïÿˆ	=.×?séS?ð$?
ý°´JR;?séS?ïâ?ïð¨)éÚ?h&"šFQ'?^¯¬,Kù÷?h&"šFQ'?ï–çüÏï ?†•Êõx‰x?ŠFÌ7?†•Êõx‰|?ïõm
?T"Ýð&Ǩ?UÍ%óÛæù?T"Ýð&ǧ3FGL J0216.4+0507@cÓH˒:ÀIà{ÃŽÀ:v¦%™½À;à€³Æ ?ÃT_Èèf±@5–٠ų@ë"ßöu=¿ãêRn·Ä¿Òë"Ì
¹¿ìƒh¯¹8¿Ø¼anô™UNASNonenone?ï˒EŠùÅ?'é—Uœ
?z6Ý:ƒ®?'é—Uœ?ïë¦3Ñ?qlxÜÒ6Ã?dYèÌ/D?qlxÜÒ6Å?î)…PÛ,f?¡X×ÀÛe?­gªòM9£?¡X×ÀÛe?ïU¨ï¨Ã?‹tX:ú‡?•Jâ
çŸT?‹tX:ú†3FGL J0221.1+6059@`³"¦óõ0¿bÿfÁÄʺÀ8Ç`‹[uÀ:Ž¬ÇsÇx?ìy­
U@ºOÌñà­@ts@i|›¿è«¶݅,¿è$ŽßE94¿ë} ÝΰZ¿ïþ¾¢ù¥ÚUNASNonenone?Æ·yF³Æj?Ăõ•áy?êR!®Se?Ăõ•áy?¡¼•y-éö?°ÚK˜ÔՂ?îä6¨m!`?°ÚK˜ÔՂ?Ú»¡˜€±?ºqè!â?â¢/p3¿¨?ºqè!â?Ǎ—ìÝÞ?±(í1Îى?ê»ÚȈ?±(í1Îو3FGL J0221.2+2518@bjª¸¥Î[À@£
ⴖÀ:LÓP0šÀ;à { ŠO¿Ç±Ä'?N¹@
³9Ó¶K?þø…à19¿îÉôYo?à¹*,q£¿×SŠ^ƽr¿äÁ¿z÷UNASNonenone?ïû³º€ZÉ?KÙRC8?A1þ"Þ'?KÙRC@?葉NÜ×?"²¼Fj8Â?†¿"lHÊ:?"²¼Fj8Á?ïlÚ£Ñ?ƒ%Rñ¸¹?ˆ¤É|××?ƒ%Rñ¸»?ïL¼!ˆ'?u,H6²(?–h{ÎíÞh?u,H6²)3FGL J0221.8+6138c@`®›¥ãSø?ä8찗âàÀ8íŒ- L;À:9GMœk?éñiþ÷A@O‹8Wà<@[Ê@«kÔ?ïþːü¿êÐÛøíDÅ¿åoKKq²9¿êõ1ÌńÉUNASNonenone0?ÌÄò<Ä?Êxà}(?èÎÃ}ùðÏ?Êxà}'?×H$·¯R?Ӎ¨N–?ä[í÷$(W?Ӎ¨N–?Öp"S"?·Rö·¼Ùk?äǵðVnô?·Rö·¼Ùj?âo : ™?Å_zÍfþ?Û ¿‹¾Ìâ?Å_zÍfþ3FGL J0223.6+3927@a¶¼œ#¸À4;>šo'À9Ì@Äì-»À;À¬ôÀ0Ý?ÙlÑYÏT<@õ"m/®C@:㟢J¿ä%,º°´¿çS$͔ɿ䝻Ýï½p¿åñè–	ŸÅUNASNonenone?îÊ¥®®Ð?©§äŒ^?£^µ¥?©§äŒ^?í*•pò\–?À2×Ü_/?¶«TxmW?À2×Ü_/?îªáÍùä?œú«V¦L?¥_ñã a¹?œú«V¦K?ë~ï±iË?¬‰"TÁ?ÂÄA:XÕ?¬‰"TÁ3FGL J0224.1-1846@hŽu:>À/ÀPÇÖ¡aä÷À:t˜XPúÀ;á÷Š¸Û¿Ë›éɁ@
Ä)Ùî@3ìŸûÞ]¿âT³æÌÓ-¿éûAÝ΅g¿Õ+s¢JSq¿ècÃUÍ~UNASNonenone?ïþF€[EŒ?6j2.§?+—úK§F!?6j2.§2?ïêä‡b7?n妁ÝV ?exÈ~`?n妁ÝV¢?ï|`¹j†±?Švíôµ?sèÒ¯)Ù?Švíô¯?ï®þ`Ȳ?yQ,ú`Ë|?"yÀgÍÓ®?yQ,ú`Ë|3FGL J0224.4+1615@c$÷QÕÀD‹·¼]êÀ:M®ƒ5ªÀ;©ãîQÓ¿ðò€Á1@±Ê]0ݘ@=½O¿äý×p·ª¿åË¥Š¾Šj¿ã.z:Èl°¿Û7\.nUNASNonenone?ïÿe¨@?Šf~NWÕ?Jÿ×ÿ€²?Šf~NW'?ïòVzzš0?eŽ§wû?[S
˟Þ?eŽ§wü?ïÃhoUÄT?|¹JßH?~KÈUÖc?|¹JßG?ïþJ-ã›?,K'°>?/;]!ÆWN?,K'°3FGL J0226.7-4747@p´Ú¤ü¤+ÀO«ud0+À:²Jj‡À;éï#8ê,?Ÿ´Ð!ƒý@
j´©ÀX@Yc_uÜP¿êzŸ6J¿é¯
Ñ₹¿æU·A ¿ãqÁt1UNASNonenone?ïø}=imR?U,ãD5"?N
ZJ·…?U,ãD5"?ïÃM•
±q?˜ø÷.ºY¹?~Y5z§G'?˜ø÷.ºY¸?îâMKDK?—ë½"Œ?¡Û+K»O"?—ë½"‹?î¶q…Îg?¡;ÒÐãÛÃ?®ä˜ç£†?¡;ÒÐãÛÃ3FGL J0228.5+8213@_"âëC-@3ÿ—þŽæ¸À:INþjÕÀ;ÖYjÕa?¼s¬h@
Èé>Èg¸@,( Z"t¿è§®K=§<¿äø'÷ŽÂ¿êë™ëñL«¿ä³°Šæ'UNASNonenone?ïʑVdX¿?'ðì<^I€?z·TÍÓ P?'ðì<^I€?ï=@¥!?¦ƒ»/ºøÊ?œ¸]7ë[Ý?¦ƒ»/ºøÊ?î¸óÚ<J?˜ÙٖUøí?¤pÂ\;\?˜ÙٖUøì?ì㡧U»Á?©é"§Ø£?¸âòÅR!ü?©é"§Ø£3FGL J0231.0+1302@c¤pâÁ*ØÀEŽ'Ð(¡àÀ9ý«®o´À;hÞë0¿ðXþú~@À…Téz@b³ ~O¼¿çV]Ÿ˜a5¿éZ^÷˜c ¿àÀIcÌ-@¿æqâÌÀUNASNonenone?ïÿÝÍ1,ž>ñ&A1rãÛ>ñgi±ƒ>ñ&A1räÃ?ïò•Ì¹ó?e 5	1??ZÔfŒþÑ?e 5	1=?ïÔ(šš»??tElýíœa?uë²²¢_î?tElýíœa?ïýf
c¯	?1ÿ:A³•?4Ϭ⇶¦?1ÿ:A³"õ3FGL J0232.6+0646@dNÚfƒÀH¿‡iì-À9öKµ
8hÀ;µ"Ô7û?ë*¬K{I@@ÒMë@SáÀNå¿çŸ?åŒü¿æf ¾;x¿íkÝxG¿ê{çNz¯UNASNonenone?ï×XÙKv¶?|¦éGq&ƒ?tS"ZD¤Í?|¦éGq&'?ï""šø\?©kx	 Ö?›¼Û¬ ôw?©kx	 ×?ì÷)ÒNª{?¨2bùcÚ?¸F±mŠ¬'?¨2bùcÚ?äLýê\"?½Î½.Àä?×f+G»þ?½Î½.Àä3FGL J0233.0+6237@`Ê8›R~@(ŠbÄñ6À9h>­º¹À:²pSO2¿ç¯`Å"i@…&ÉB~«@XL jÓ¿èl÷òaÔ(¿ç˜Oº}iã¿ì×1ú™¿ØÃîÓTUNASNonenone?î3â¥úlŠ?°juí]'?¬ÁÕ Y7`?°juí](?îсX9jj?½!rO?¢çê|iYQ?½!rO?éÖcEØ°?²×¯Ê;!?Ȧr鼝=?²×¯Ê;!?ïó%¤(²?W582»æ?XÅ´·®™Ý?W582»æ3FGL J0234.2-0629@f-ˆ¤~ÏêÀMf^ê–À:ëLÔÉÀ;ÚY§;BÌ¿È´• ˆ³@÷;á,«?ý¢~ðuô¿ºô¿§¦€¿æqô%‰Û?Ÿ÷*|'T¿Í†•'˜UNASNonenone?ïþ‹¢ë{?-0Lÿ!?'EÑN\œ?-0Lÿ?ïô}0Çj?c]™ù+¿W?W÷žq-ï?c]™ù+¿Z?ï³Eúñƒ‹?|15•''?ƒ.CŸL?|15•' ?ïú =¯?A!c×¾U?Eë	CÃ?A!c×¾M3FGL J0235.7+5647@aC¿rq7À	Þ×ü«·©À97BL«ª=À;KïW;P8?žô¸[ö@nȯ†Á@Û©Àƒ=b¿ç}D®-¿å¿SÞµ"±¿çÈÛ$¹=¿ìñډŠUNASNonenone?íÓ¯«eF?´®ÛŽ‰ô,?±b'§$ÕÑ?´®ÛŽ‰ô,?êèþ}]I?Çõ
ø‡»?Ä\
ŠÛ–?Çõ
ø‡»?êÿ¦†zÝ?²(Osp?Äeæ‹'?²(Osp?î]—C}ï?—è)Íb…t?ª&ŽëÈ!?—è)Íb…t3FGL J0239.0+2555@bè¬1&éÀ>ö]9–úƒÀ:"Ë@ÒÎÀ;Êry\ã¿ÛºI˜át
@
[,µ•£–@~¸`¿é)I8òԍ¿è—›‡…¿Öïòª	±ã¿ÖaÀ~#¶UNASNonenone?ïÿÆj³>A?&¯ÖXj>üʦ`ßç¸?&¯ÖXjx?ïæ+0Ö:÷?sSß
9?iÔÏ)Å	5?sSß
8?ï×+uÇa?tà"gìL?tjE}O{?tà"gìN?ïß]›¥"?hpö¦7ý?pQ2-6R?hpö¦83FGL J0239.4+1326@cæ_ZÙjjÀDÙ5C®«zÀ:
¹üæpÀ;¡ƒB??±¿îÄ×,n•V@v­Aí
Z?ÿìe¾ö [¿ïMQ'Ì?áÌD' ñŠ¿ácH7¸dF¿ãwrt³þUNASNonenone?ïýßfH#?YZ>U¸©Á?1;çT¯?YZ>U¸©¼?ïíÄX•?mфƒãݓ?b;§jâ÷}?mфƒãݒ?ïÂ:ž²õ¤?y0–Dí$?~â°¦….#?y0–Dí?ï÷ ð¨á?S#½eêMK?Q¾¯ø=¸?S#½eêMH3FGL J0240.0-0253@eÓ0üø
ÃÀK>ýuâlÀ:T¢Bµ‡6À;ä™/ŽÃ?è™SèNL@­Ô°p÷@€Ì_iœý?ϧïâj\¯¿çWvÜL¿¿ïÔFxVË5?ìý["KUNASNonenone?ïþYŸªdp?6Šž#'µ_?*fY¹Ý?6Šž#'µc?ïóËjq?c«Ç…Çz.?Xi+Í÷q?c«Ç…Çz/?îX;
l?›Prµ\NÇ?ª|O)>‡'?›Prµ\NÄ?ïìŽ+Ëј?sÕâSÉ@4?cqÔ4.hu?sÕâSÉ@33FGL J0242.1-0534@fS—c^t*ÀKûà¤&À:jùYó']À;ãåÇo•º¿ï²	Û~Ÿ@½§¹íÍ@×è€\†¿¿é`eŠÀ°+¿ä.ðÞ¤æ¿âTÂÝé2g¿ïÿZ=†UNASNonenone?ïýq£Ù??…§ia?7¼rá0m??…§iv?ïñ;ô?g+êÂÕZ?]òe'ú?g+êÂÕZ?ï,VBu8ç?'Ó¿\{?šu7±Xã(?'Ó¿\{?ïùË4¤\±?Hy^B†$¦?HÓ-n;g?Hy^B†$ž3FGL J0244.4+4745@a»C¬ÄðÀ%Ø?³t63À9ە+uϐÀ;©V)Ø@ž?óƒ#Á%NÄ@]¦^y(@þ€[¯ÿ¿èN›c?·È¿èÚç¤m¿í'<«WL¿ïþ-€IoUNASNonenone	?Ó8ìªú·D?ÐÂx‹««?æc‰ª'¤^?ÐÂx‹««?™éÏ=·'?®÷‡¿?Ä?ï0±†Gw?®÷‡¿?Ä?┃þÚç?¶€yÝæ,?ÚÖøüJ2?¶€yÝæ,?•ïÃ0ÿN?ˆ+ùŠ8g?ïPçx?ˆ+ùŠ8h3FGL J0248.4+5130@a™
9À<ù…'À94´7ª'À;Oº*2Ùq¿Ð籺¢¨·@ûD¸Ã+@‰gÀ-­?ÆáëRôš¿êEØU'_ü¿¼e"¤7,¿áW£UUNASNonenone?ïÀÔë??Šûå‹Â~Ø?•Š`r÷z?Šûå‹Â~Ù?îEüyN{?¸£wkƒÔ?« 8kO´?¸£wkƒÔ?î¦O&úGx?›*ÝÅ¿FW?¥›
[ˆ…?›*ÝÅ¿FU?ïuæ?ç?_Ì'R?']\8ú?_Ì'R3FGL J0251.1-1829@i;ºKâÀN•6½+oÀ:¥?CÄÀ;Ã}ºŠ?ìG>^ú%9@
b›«—ž?ùëÿ0ø?ïÿ9Ã^ÿ¿ïÿô	N*?ïÿÀ¤Vt¿à¡âDrªUNASNonenone?ïþÃ৸?)`wÅU?#Αõ"ˆ¶?)`wÅ`?ïï
áš4?{‰jeà"b?`òeËé"?{‰jeà"c?î½Õ`–2…?—×÷Þª]?¤"©öœ×¬?—×÷Þª\?ïËÕëó H?œ*síÿ¯"?z
/Ûð?œ*síÿ¯"3FGL J0254.2+5903@aDèh3Æ¿Â6év&À9Rk–QÀ:Õf££×?w0Éraˆ¼@­ºÛ³šw@D¾@Bo¿ä¨ÞI昿ë+`Š.m¿íµûxT?ÔÕĀ€¡"UNASNonenone?ídšÒx?»ÃlX	L?´ß£)l?'?»ÃlX	L?æn~	ë,«?Õøš©Ö?Ó#ì)¦«?Õøš©Ö?é:  ª|?¹%e+?Ë}Wö?¹%e+?ï¶uÆ
2?…ý[sa?'bŽ|³{¹?…ý[sa 3FGL J0258.2+3555@b¼§›ºÜ
À47ÙUqKÀ:({_ïJÀ;¯è?ïÚÀÓ$‡É¸p@
†ú·Šñ@àÄ *í¿¿éÃG†Yÿ¿ä {Ó·'¿ïûbd¬°€?ïÁ˛R	UNASNonenone?ïôaéO?c‰T8J–a?W=ð-aõÑ?c‰T8J–`?ïå0ƒ™Ô%?y›³Â]?jÏ|f+ۇ?y›³Â\?îÚ¬qäú¶?"÷Yƒ/Ë?¢U8á°T¦?"÷Yƒ/Ë?ïÿÿþÉ5>@oUC>#l§ü>ª¤>@oUFêX3FGL J0258.9+0552@eW¡"úÖËÀFk	cV®À9¶3ßWÀ;†!È`?ákÒ]Ä_@
KYN$ü@ÿ9À@!ƒ¿à˜[êȜx¿Ýìß@0¶p¿á+µ¹=s¿æÛì4£"UNASNonenone?ûْg?‹ñ˜Ý3Ž?ŠÒ	›f?‹ñ˜Ý3Ž?ïQ>¿±•w?cWó°ð‹?•Ø(	ÍQ?cWó°ð‹?íê­;óô¸?¥¿àëzNð?°ª– `Z;?¥¿àëzNð?é'õ?©ˆ@ K?˕µ¼+‡Ü?©ˆ@ K3FGL J0307.3+4916@bAcÀB@TƒæÀ8ö"#—µÀ;KÒ®Že?Ù¶ˆ™'j
@ÕwQÆX@ÄÀ¿¿ãתˆ+µ¿Ú"ì¨y?¿åʖ;T¿ØË´¨'"nUNASNonenone?î\'mH?§mžÀ4?ª=©.+?§mžÀ4?ív'€™ðÝ?½7©JÛÁ?´NÃû0y?½7©JÛÁ?ìGÁ‡?¬Ÿ§Èmm?¿-Áñë"Á?¬Ÿ§Èmm?îÊ ðê?Ÿ1ˍ7´Å?®#Uðþ±P?Ÿ1ˍ7´Å3FGL J0308.4-2852@lÀ6âëÀMèÀh ÓÀ:Š7"D[À;õ½
·éç?Ѹg¡5+@
¹õ¯š@Kª@ýÁ¿çCr-nù¿æ&ÓØš¿ÚÀÇ2p¸¿ïÿNµxOûUNASNonenone?ïó40׸^?i-ô-T)h?Y—žPD?i-ô-T)k?éÙ#:E'?Í[å¶fú?˸›së`?Í[å¶fú?îšÜ&ÓÍ?ÜVF§…À?¦R=ŸÂÃ9?ÜVF§…¾?äŽv‹.çÏ?Á\ы‡?Öãé¢0d?Á\ы‡3FGL J0312.7-2222@j‹†DR?hÀL×Y‰ßsÀ:h©ÒÌÁÀ;µÙÅٔ?겸›VL@ ¯Õñ
Ê?ùÿ¤ÐÚ?îR'äɘ»¿Û¯ÈqÀ®ÿ?ÖáëxşÿÖÃò™Ì*¢UNASNonenone?ïôöll ?W…
Öóš?Vé''¿Ý?W…
Öó ?ïð/ læ¤?h¨ŠÒ?_ ¿&2¹ ?h¨ŠÒ?ïrlWã?"Pîg"­O?Ÿ1²uØ?"Pîg"­M?ï¦ã(Б?«ÆÈZ7¦?†G5þKۖ?«ÆÈZ7§3FGL J0312.7+2011@dP¿Ž`€À?›Gb• ŽÀ:$o±hÃ8À;—¨=¡K?¿ÛÃ5#Î;b@XšJïg?û_¿^Õ¿ïI;Ø?áßN¼sÒ¿ÌЊqˆƒr¿ÓÔÃáÁ¦~UNASNonenone?ïÿs'Ê8?[{KW~Ã?¦¸íß%?[{KW~¼?ïë¡l¹Ø?o\þI-¤1?d^"üF(?o\þI-¤2?ï×=$‹?p`vâ¨|c?taqíºww?p`vâ¨|b?ïùárq1m?DË3—ô±?Hz6;:L?DË3—ô±3FGL J0322.5-3721@n¾"åÞÀLY@_k bÀ9õM–ÃüÀ;ÞGòù?å>k¤Ø€Ï@.:âT@™* :8?Øj*ÊȪm¿âÓ¶Gnj>¿åß5C}n¿é'l8YÛ
UNASNonenone?ì9eÈLl?¼»2WS?¾4ѽŸ£?¼»2WS?îî¾ZÛë|?¦ª$§l—3?¡RAH>?¦ª$§l—3?êp›•'œ?±å£Jáû‹?Æ="Ñ©µ?±å£JáûŒ?èÒ1_Ñ?²ð8˜mŠ?Ϙ·:€»Û?²ð8˜mŠ3FGL J0323.7-6038@qB¼£n/ÀGç4.ÛµžÀ:|#²Œ¯¦À;àÖìá?K¿ûð ;´·@j‰9Ðf@"È߂\¿åy3Ѥß¿ì¬\`ÂÒ<¿ DÏI'¿ïÿ·`²zðUNASNonenone?ïþ¬ƒœ
ˆ?A®¢á–oÕ?%7Æ?Wz?A®¢á–oÑ?ïób'ãÝØ?dç< Zõ¿?Y:ú8DOW?dç< Zõ¿?ïÊ]²%?•ôg1nö'?œæ´I»j?•ôg1nö'?ïÿÆAšq"?
µܟ>üß2Ç>7ì?
µÝ3FGL J0324.5-1315@hï?»×²ÀIÖf¡ÉÀ:R\±±¾TÀ;Ó&
UÄXÀ	rö퇭^@
†Nž)Ì@,è…Ç*¿âÁEiãì¿î¿æ¬¿3?kîb†£k׿ïÿ¹±3ŒUNASNonenone?ïúÖn˜Ú…?bµ#Fò‡
?D¦Eœ•ëh?bµ#Fò‡
?ïôXc×?dqY»´$ã?WO9ÝÚPî?dqY»´$ä?îº.ñÈ?)ÖlŸ-?¤]Äã~Û?)ÖlŸ,?ïÿü8&>Ö¾Ôu«L>¿î?îÐg§>Ö¾ÔuªÛ3FGL J0327.4+5828c@aÄí(Œç?øÝÈgã>(À9vG…À;ûXÑRn?ï0=÷(ã@Âg
€F6@•À8–¿ÙÑiüÀQâ¿å®üd¿ó ¿ì="ßEu¿æÿBpÆoUNASNonenone!?âÿ›]® ?΁l^@?Úx€ÉD¢Á?΁l^@?ÎHi¯A°?Ð;ÓÀ¦µc?èmå /"?Ð;ÓÀ¦µc?ãI¯Ûeç=?½Uö8[£?Ùl I41"?½Uö8[£?Ö§ö™aû¨?¹¸ˆ³?䬳O+?¹¸ˆ³3FGL J0330.6+0437@fp¯%;ÀD]9–úƒÀ9º~¸lÃxÀ;'ØåßÃJ?ìJ	
šÈ@|Õ@8Õ@ä`RP/¿Ï¹2À`qŸ¿äÖƄDƒú¿Û[kP…ÿ^¿ïÿðH°{'UNASNonenone?ï/‰«ñmD?¤ÍF¶?šʁÒW|?¤ÍF¶?íÐI8³Mo?·ˆßKc?±}¶:e"Œ?·ˆßKd?åíB˜‰å?·ã¿>Ôü?Ô%{âÎì5?·ã¿>Ôü?è<0}9žÏ?·
ÝÈuA…?Ï>"Ä?·
ÝÈuA…3FGL J0332.4+4644@b¯a¦
EcÀª	EùßUÀ9®?uŒÀ;k|Ìy1?í[µ‹Ás@
c?aì@À}àU•´¿á±²-þÛ¿êŒtª7e¿æËirµT5¿æ»Kô
˜UNASNonenone?ìŽüd:?¹BØ
'hD?»"Þ-?¹BØ
'hF?áñT¾}'?Õhɝ'ì›?ÜxVƒú?Õhɝ'ì›?éU•—_¯?´€†0<ÑÂ?Ê©©¡úB?´€†0<ÑÂ?Ù¶Ÿª—è…?¶a‡Ýxµ?ã$°*´½?¶a‡Ýxµ3FGL J0333.6+0233@fÆÝ/Ÿ¾ÀDwŽ`€sÀ:;à5_]^À;»*‰@†¿ðÏpˆ©1g@
+Ž
{"@'vŸït¿ÜÏ?ѯ¾'¿æ~øù?¿ÇÝ0r9¿èæßé<͙UNASNonenone?ïþv³öÀm?,˜7'FJ¾?("À"ù<…?,˜7'FJâ?ï˚/?j¶•æf?af\4eц?j¶•æf?ï/ž<ÐÆ?"™|Gæ`ò?š=XeçT?"™|Gæ`ï?ïûý?Ei	ûA¿=?BÏóûD?Ei	ûA¿;3FGL J0340.4-2423@kQÃóà7ÀJÆ)ñkÀ:œ+Àx*´À;ð|_Ìï1?À¤7F,#@
'Ù@µ/ßì5¿årekÐĺ¿Ú0—–£ß²¿äÀ9EñÑ¿¿áð™#ì³UNASNonenone?ïòqÚë+?^ÜþmAÃ?[Kâ)ªÂ?^ÜþmAÇ?ôT'ú?œ¹£·!Ð?ˆÖBêہj?œ¹£·!Ð?ï/¹¶|æé?·Í(=‡ˆ?šÉ0c"ä?·Í(=‡‰?ìÆ)®s
?¦Ÿy+»Œw?¹Î²Œg¿°?¦Ÿy+»Œw3FGL J0342.3+3148c@d
â'@·€À2a"D¿À92»K›	À;,äd™?íϣԅþ²@ôÑø/Ò@5F@V1e?ïã–>§×¿çA½¦ˆÉ¿ç*éy<;¿åGÅ	›‰UNASNonenone0?î6^ñ‹Á7?µ|›B'\?¬šçCì?µ|›B'\?êó­0?ʄ»4(ü^?Ä3ý½K?š?ʄ»4(ü^?ä'ùGVŸs?»NࡸŸ™?×°
qRÁ?»NࡸŸ™?àSzÀá7?À#§Î[³Y?ßýY
~='?À#§Î[³Y3FGL J0342.8+1321@eƇçÀnÀ?÷\9¼º0À:z¦ª#T™À;¥ôæò?ä0ÈCiûá@
LØÑÞ?þ‹¾_K¿ò?¯&ˆÀXu7¿Ë
ùЈ¿á®ä^ä¼Ù¿ÞO•vk¹"UNASNonenone?ïæhñ=°?m´)PK1C?i—ÂàO?m´)PK1H?ïÂîÍ-H?Šc®ë 0?~ú™i[Ú?Šc®ë 0?îޛˆ¶Ðq?"ÊV¸!?¢Gt'øñ?"ÊV¸!?íõ­u?¡ØI˺Àß?·3ðR"WY?¡ØI˺Àß3FGL J0348.1+4431@c!Ù©T"ÀD=F²lÀ:;ÔÂeÀ;n=)HÏ?ºŽ›t÷4@-}ns%@5G zô¾¿×¥Á'~iµ¿çÑÚ?üð+¿èduØÊ1¿ÔDRû$¤UNASNonenone?ëÉíÕµð?Â}¡Ï'd?ÀÛìH©(>?Â}¡Ï'd?ëÐ(dü«'?ÉeàÉCc?À¿^l
Q¶?ÉeàÉCc?ëo.ë"ñ=?³ëÌޙ+Õ?ÂCDSt;	?³ëÌޙ+Õ?ìȹ·%ÚÊ?­›—¯F?¹º2FÑ)²?­›—¯G3FGL J0348.4+6039@aßî$5in@‰Ð~25À:2‰'
ÙÝÀ;± žÛù¿ÓLI¦@
^'í'úÇ?þ4A%9J?ïþ"¯OÖ¿ëÞðQJö¿×<•ì»Ö¿…8…âÀo•UNASNonenone?ïÿZÈC
y?û¦?×(?¦÷žPï?û¦?×
»?ïÉÊ4`-?ŽÁ.Lï»*?{uåÏé?ŽÁ.Lï»)?ﺓÓ,3?{U^ü¢"a?[4ó Œ?{U^ü¢"a?ïùø>á^?Fþ‡ö8?IÈz…ß?Fþ‡ö83FGL J0351.0-2816@l,@N¤©ÀI:žË1ÂÀ:½4Ùü`8À<ßÇ{T4¿æÛL@
1S1€U¦@WL_ª	©?ëB³ÔáÌ¿ÜÎÊÕô
K¿ç-@µ‰˜¿Íp³G%ëUNASNonenone?ïí£ãÒ?fúå"Áê?bþû\-ñ?fúå"Áê?ïò+×P?e^ëû‰?[¨Q_ÍN?e^ëû‰?0¼?¡?²õ
û?®Äuüþ4;?¡?²õ
û?ï÷êúQ?L¦F~ßÅå?P*
ß]í±?L¦F~ßÅÚ3FGL J0351.4-3248@m"ßÎ1QÀIs,B»fÀ:eZJÏ1+À;õ¯OäCâ¿Úp6Úîµ@JÌõfžð@`g "I׿è%¯ó´Sj¿ç=‡ëlm¿æc¨]¤n¿ïÿê†úŽ/UNASNonenone?ïþß/–™?1HëBvp?"
æ–y¾?1HëBvo÷?îÛîC.o?³.é™.5?¢AÍ?³.é™.5?î­oPÏ?–wÕl[º·?¥/žY
ó?–wÕl[º·?í¬ªÝ"úß?¥ÍªïOÛ?²š©Ø)?¥ÍªïOÛ3FGL J0359.7+7649@` Âø7´¢@1ÐWÙÛ©À:¥ID°FÀ;þb°Ï@E¿ÜôP‰Û5›@ñvæ;^@Sù`(´ª¿í,#³Iª)?¨,ôÝ¿ä8B¿è‰¸Ÿˆ	éUNASNonenone?ïïo
¯ª?dRe5ä³?`põPU7?dRe5ä³?ïÌ·ÀÑÈ?Ú]öÒM]?yý$—Q?Ú]öÒM]?îÖܛ6›?šh¶	~ù?¢'6O̖T?šh¶	~ø?ïÙì§<=ü?nYíÜA}?s	¬aá
?nYíÜAy3FGL J0401.0-5359@p'4'¾‹ÁÀG'.œË}AÀ:ÚºÊkÉ}À<:L,(}?âׁα¾@Ý"bô@ɑmä	¿ã8Ûn®¼õ¿è¤ÐÌX*0¿æŒVöq€?ÒPJ¹?YæUNASNonenone?ïî!oA¶?kí;×¹âU?aÞ搾I½?kí;×¹âW?ïïAþvE?kè{ˆBP?`¾ñ‰»b?kè{ˆBQ?îË¡ûª;?¡Š­v8?¯³EàE\H?¡Š­v8?ï"Ätî…?žmn«žT<?›§b/h?žmn«žT;3FGL J0402.7+2616@døP›ùÆ*À3"{՝VÀ9Ó÷Ò4ÛÀ;'‰¬¼Œ
?—½Iëêý@\ut cM@.Ðg¤T¿èU‹ûÝm¿él"©¼¿å'Ó¾¬¿ïþ[híxUNASNonenone?ïÏCÚXÆ?€®oœ­Ž?x^ÓôW?€®oœ­Ž?í¡u'n?½''ÿêê?²ôWÓº?½''ÿêê?îõ,¾‹A×?•ßÏÓ!? ­4Kâš?•ßÏÓ"?í¤ekc³ª?¡)yÃ
ˆ»?²ÜÔ¤âb­?¡)yÃ
ˆ»3FGL J0412.0+0229@g³ÞÊl À@¬e"¯OÀ:
㎰1ŒÀ;'Á.32¿'-Q^·ÿ@V±Ÿõ©@0oß`ù¿ç	mý^¿àŸÁ¿ìšr
±¿Ë×2®uk3UNASNonenone?ïíIª)³?k\AT)|?b¶UðÖLç?k\AT)y?ïëýu¦Î'?mS—Ðás?dŠY1nµ?mS—Ðáp?îÒpm~¦´?™üIßõû?¢Øù("«?™üIßõû?ïã˜Ø³?eº=Ύ[<?làg'Lse?eº=Ύ[:3FGL J0414.9-0840@i;0©7 ÀCMs\.ËÀ:4õIØqÀ;Ï$Ù¸¿æ{ÄА7@ÚAP'Ny@:³ɹȿåªñ)gFO¿å¼;÷k˚¿áû&'ÕŸ¿ïÿ½¶¥UNASNonenone?ïÿ"ç½1o?&Q SÓ3?£YÒ
.?&Q SÓF?ïâzÖT?vœ™Äh,?m…ü)«.?vœ™Äh,?îöÆ>| ?•îEÄZ-
? Ÿãœ5ù?•îEÄZ-?ïç~T?eRcÛï/?hìþ«ñ¾?eRcÛï03FGL J0415.7-4351@o#zcslßÀFý<£}šÀ9þ¥é34áÀ;ø½$¹í?Ûytß꥕@
T—'hÐ@݉ÿ󕹿àe¸Û[ä¿çŒÁ!¦v¿í.	öV'¿³9¼k—UNASNonenone?îžÝÍl?°á$ìόÜ?¦#.‰?3?°á$ìόÜ?ﲔ¸W"?õøÄ?ƒZÏQê-?õøÃ?ìv¢'?ø?°Bxü6ó¡?¼Oúëî>?°Bxü6ó¡?쒤fÙ­d?´5õ  °?»jÜÉ2"×?´5õ  °3FGL J0418.2+3412@dzxl"hÀ'ǟfb5À9ÿ9¶ÚóÀ;…vfŽªR?Æîê['Ê@
íyøêb	@úg–
H¿â:|l{íü¿ëÞ0Ss´G¿§¦¹—Úµj¿ïÿù½p¹QUNASNonenone?ïÁ¤ÄÀš?•¢ÇXa*?-·Ÿ³$?•¢ÇXa)?í4
ô¸Ä`?ÁVZÁø?¶_¨Z9Üú?ÁVZÁø?íÚ¥>ó¹?¨ÜŘ%$w?·¡*Öb/?¨ÜŘ%$v?îñîö9ô?¥¸Ê'à? ážì`¾?¥¸Ê'à3FGL J0419.1+6636@a±+Iº@'#póˆ"À8åbøÜ°À;e¤ëàŽ?ê§cۋpP@(ÛèH©<@~@Jª¿âÎð´f,¿áލf_A¿ã°ŠÕd)¿íþƒŽ¯UNASNonenone?Âað‹é`S?À>½?,ZÒ?ëgƒÝ§ì?À>½?,ZÒ?Å	Q?Ê@ywÌ?꽫¿:}9?Ê@ywÌ?ÕRú¿m"ª?¼2qgՎ«?åV' I=ª?¼2qgՎª?̍Ž¿ÖPµ?±šÃ¿?èܜP
kÓ?±šÃ¿3FGL J0420.4+1448@f|Rç-¡#À87:G#«À9µy1DEªÀ;TÍè«P?êûˆnp@µÇ'`@î¿ÙtP¿âÄMA§?J¿îŸ<=?¿ï"¶|d´?äaU¬žÔUNASNonenone?ïž1»nN?'ÇW¯*í?ˆs'$z,Ç?'ÇW¯*í?﵆¥+!?¤lËmCD=?'žV»õ7ø?¤lËmCD=?ì§0™Ö¦?¦ó]"æ֕?ºÆ{1JÏD?¦ó]"æ֕?îúg–?¨ê*­˜_? Wîɇæ›?¨ê*­˜_3FGL J0420.4-6013@pò~|áœÀDäcÇOµÀ:—Ì9ÿÖÀ;åï3ÿáÍÀqãá'Tý@
š%ۆÎç?ý†Jßø"¼¿ìCÉ»A×]¿Ä|øƒßÈþ¿ÞM±Ôx蟿ÔkËCØUNASNonenone?ïþ÷5³k…?è$ÃËa? Œ¤ÉGµN?è$ÃËG?ï󃉇»?dÊt—¨Î?XøìðˆÆq?dÊt—¨Ì?ïÇžQ0?wzyii
B?|0ý×gì?wzyii
B?ïÿû¥q{>ÑÇ`rÂ.>Áj;öu¸>ÑÇ`r¾¨3FGL J0420.6-3742@n	E¶ÃvÀF˜#πÜÀ9[x̚xÀ;£Š:?Ón±Ê¤@凖ŒÉÒ@®m@ .3¿å?Æ ¿ã>ÍI¼ä¿ç†ÍmËNa¿âäӏðµUNASNonenone?ï֘´âw?…±ê¬%?~4³¥ŽÄm?…±ê¬%?ïÜvé¨'Á?~¥/­™¾[?qċ+ìq?~¥/­™¾]?îZÕâ7\?¡MAdžð‹?ªR¡Þ̊K?¡MAdžðŠ?îMÎHßGè?—Ûú*Q™À?«#r?—Ûú*Q™À3FGL J0421.6+1950@eýR½<6À4¿ÉGNÏÀ9œTŽ†@À;]¹û8ðâ?ãø­âb@Ðf{Š
@¥ã€B…Œ¿ÙæÒ1¿æ}ô}s{Ö¿âö@O6°'¿ì–­™*ÞÑUNASNonenone?êNß½Ø?Ôb"bæþ?ÆÇè	øŸ?Ôb"bæþ?ìÌØcu?»ôÖté9Ê?¹Ÿq<äS?»ôÖté9Ê?è:èŽ?´Šuø›÷¦?Ï_ÍÅ¿Ñ?´Šuø›÷¦?èƒ\ùL?°‹'N+°;?ÍóƌÏ ?°‹'N+°;3FGL J0423.5+5442@bϕBC@åœÝøªÀ9ü*ˆjÀ:'Ýr6~A¿±-ä?GM"@§ÃÓÔÔ@™€D3¿ãº¥¹ëý¿ìî­…M¡¿Ñ8Áïñay¿ê\ôïøîUNASNonenone?ïÅÚ£€J?ˆ«úvü^'?}®?Ú¿)?ˆ«úvü^'?ï¼b¥;ž?'=%ôÐ?€çxV±‰?'=%ôÏ?ë?8³69Ä?­ŒEÑLik?Ã3'ò?­ŒEÑLik?ïỐåÊ?sÚµb¥WB?nDo5è½?sÚµb¥WA3FGL J0425.8+5600@b¸"t¼j@d‰Ø[À9ƒ!
–ÁxÀ;
¤$7îÀþü¯ég7@=ïN×Ô@Çç^j¿çü(ˆÆsÓ¿éäÅ©Re¿åa9Uâ	Ë¿ÇýºDMÒUNASNonenone?ïðóã*lo?dv¨zb6]?^9«'"ž?dv¨zb6^?ïÐ=•-¨?ŒÞV1…õ}?wáuµi,?ŒÞV1…õ}?îmËs?£ä;€p?¯.ƒOÑ?£ä;€p?ïÿó¥µ;¹>å† u˜m>Ø´•ˆŒºŽ>å† u˜³3FGL J0426.3+3510@dœP	,ÏlÀ#P—ÈAîÀ9¿Îí8}À;.6Dÿä?ë+ܱ`#›@À;#°@èÏßüª`?ÄE¤—­¿èäKGbPh¿äE"‰£ñü¿ïÿô_
ÄUNASNonenone?íà‹nVÞ?¾~?Ò°R3?·ˆû¤I?¾~?Ò°R3?ÐY	ÙÙ9Z?ι#¨l?çÓ{cR?ι#¨l?äò0)Ƭ?¸©áýÞLÞ?ÖñŸ¬r§?¸©áýÞLß?Ò\WwU
?´‰b=Ŭ?æÑÔDtU{?´‰b=Ŭ3FGL J0427.9-6704@qr(õ\ÀCE±cºº|À9cGK,GÀ;Óêçj¿ÜùüP¸@
‹ÝT@¨`ÿŸ2
¿ãõ趧
_¿çt>!½ƒÈ¿åXbü"RÇ¿å\{&kUNASNonenone?ï'ø•Î9¨?–«IS¤†T?‹Aڌq–?–«IS¤†T?òöX?·Í–øðÖ?¥'@К~O?·Í–øðÖ?ípÜ'P?¤¼†ÍÛ ô?´yçûu?¤¼†ÍÛ ó?î]'ÕR"?¢oèarÍ?ª.'ªÝá?¢oèarÍ3FGL J0429.8+3611c@d"ãû½{ À ނ/ðˆ"À9vygÊêÀ;õÊ?ìms†"
<@
¼¹"EŸ@üŸÀdµ¿ÕË룿çå#üg!Ö¿áÎ+uéU¿ïÿÖµdUNASNonenone8?ãv!ÓÍÛ?Ñ+«Ü€Ý?Ù¼YÊdJ?Ñ+«Ü€Ý?Ð9=*Ir?ÍúD& 	?çãavjÛH?ÍúD& 	?à'ß1?»'N˜5O?ßÇý±ÀAž?»'N˜5O?ÖTɯøŠ?¸[Ã&Rê?äñ՛(º?¸[Ã&Rê3FGL J0430.1-3103@lìÞÊl ÀED¤Ò²ÀÀ:°+Xs^œÀ<
Å󔷳?çß™3©a@LzNP?ÿ‰ÀGƒL?ïý-óáÂ0¿äéö[ïó¿Ë:B†M[¿í€.ž*UNASNonenone?îÒ4õ©ÅÛ?±"ä4Ô9¼?¢Ü°¥c¢R?±"ä4Ô9¼?ïúÊáٗ?«s#Z?ž€¦£ÄÍ)?«s#Z?é'÷•.F?³X÷@f›?É´!«Fçí?³X÷@f›?í}Ëïf?­æà¤Xýh?·ô) "Å?­æà¤Xýh3FGL J0432.5+0539@g¿—$tSÀ;ZÀh ÓÀ9ŠDZ¢ãÅÀ;Y»JÄIq¿ípƪÚð¸@Pèà©£@ŽÝŸ'禿åëô¿íU
:ç׿×ÞÞY‰€"¿ã"+Ù-ÆUNASNonenone?ïÿ…‰º?óšÆ'?¿x'ƒ?óšÆŽ?ï苣AË?qš³È{…?gt\¾ø5S?qš³È{"?'Pž?‡Pìï*Uß?ˆ•kߘÔ?‡Pìï*Uà?ïüuAø?7Æ2—ß:À?<U÷{€:í?7Æ2—ß:±3FGL J0434.3-1411c@jWŒ½D¦ÀB[hœ¡‹ÖÀ9ñƒ 3ÏÀ;œ£©½Ô¿é •ìÄm@ü'ã@Íÿ|wu¿ÛÀ)˜œ2¿çÚý<´ÄÌ¿ï"ÿž'À?áv×fJUNASNonenone!?ïþR×Ò>f?2?/ο ?*҂܈x?2?/ο ?ïðÈw¢œç?h#Ü`ò…@?^oºÆ2l?h#Ü`ò…A?63·?™â[×ÓÂ?¥¿Ö,œÄ?™â[×ÓÂ?ïÿc¹lɺ?oŒ¡]/?ˆÒfțh?oŒ¡]3FGL J0437.7-7330@qá[À6ãÀA˜À½ÊÑJÀ:6`áÂ'WÀ;Ô}Qœ?Ú:¿ö@ý
WFã¿@Êß^Iâ¿ç4ãöERV¿éæ—S™/<¿¦·äüLð¿àÓ´[x	UNASNonenone?ïÿµ% ê?%¥UÀÔ#?¹6—ÅTf?%¥UÀÔ¥?ïéï¸Óc¢?oä9ó@Œ?fG,œ]ª?oä9ó@‰?ïÔÌ6	æ?uíÖ÷Á}³?u™äü{‡?uíÖ÷Á}¶?ïÏ!#I?sÏ;ªä†?xon[7þá?sÏ;ªä†3FGL J0447.1-2540@l3E¡ÊÀƒÀBØò{²þÅÀ9û=5´ÃÀ;ÓFóÚWпâɽé…Q@
>쯖0.@ÅàŽ6¿å<Ó@Àu¸¿æTþ&¶øû¿ç;M—ý& ¿è
&S?±àUNASNonenone?ïø೫Û?R£l5
(?O˜}1P'_?R£l5
(?ïÆÛ%&)F?ŒßxmÐ
?|'mlë]?ŒßxmÐ?îñs5µo?"Ï5?Š±l? è̤©1?"Ï5?Š±k?ï‰Vz¨b0?ƒÛ)¸
N(?ªaUçt?ƒÛ)¸
N'3FGL J0451.6+7231@aXÓZ…‡"@1‹Ø¾r–öÀ:F–À¡E`À;Օsš+?æ"+de@
فÞç×j@5.?Ù^Ö¿ê7þ¥ü˜0¿å/–¼¿Þ0‹"iAô¿ê'/îÀ_UNASNonenone?ïÐG;m{?æMõ õ?wÜbqÉBV?æMõ õ?î'Æ–ôü?®…âò½'Ø?¦Ó––ð°L?®…âò½'Ø?í¶jœð1?£÷ѲªÈq?²L«~wP?£÷ѲªÈr?èð¤óêM?´v`%#Ó?Ì=l0VÉÁ?´v`%#Ó3FGL J0451.7+5722@bã©æî·@ £›ˆ‡"ŸÀ9¸ÀÂÓNÇÀ;n:©I:?ÜRVMƒZW@
¿Ñ2œ_@䜿¾ÇQ¿ïµoŸf&?ÐXÞ_闿ÕÚ`:Ê£Ÿ¿àèaÓ¯•UNASNonenone?ïàÑÃÙ×?u!Ûò˜H?o.í<&(a?u!Ûò˜H?í±\Û4lî?¾Å'0n(d?²u&\˜"?¾Å'0n(d?îFиäò?ŸÁõX›1G?«'ôq°ßÈ?ŸÁõX›1J?éÂúã¬-?µ$!v-ÿq?ÈôÜqOL?µ$!v-ÿq3FGL J0456.2-6924@q‹öy|ÄÀA¤6~ANÀ9fÁæ¯ÍÀ;ŠCV–åŠ?ôUü¬
‹@!ÓÛߺ:@vQØ7?Í6;9¥¾¿é¢<²I$¿å`î¦L–˜¿áB#hºÔ}UNASNonenone?ìE¶ê(&N?»W­¡ ZÔ?½ÒH®¾Í–?»W­¡ ZÔ?î"°Tó?¶ô¯·)>'?§¸"ú°Ü?¶ô¯·)>'?èhј‰7?²§ґ7?Ïú\¹Û%?²§ґ7?áihçÅ?À3ªmé4?Ý-.yÞ°y?À3ªmé43FGL J0502.6+1759@fö©ûçl‹À,~$5inYÀ9¼R¯Ð<ÄÀ;@½½eP½¿øŠÖ/¢!@˜‰°B}~@TZ 4"[¿àɪÄöOä¿í¢ý††Ÿõ¿æb"9éŽW?ÒZðiÃUNASNonenone?ïðë"pf	?eGã
?^)»3î?eGã
?ïØÖrNb'?Š£zý…?s"ÆØη¥?Š£zý…?íû5Œ_Ui?¥½¬'GÞS?°&STµ?¥½¬'GÞR?ïÿáòLì)>òq51–d>î
³×j>òq51•Ï3FGL J0506.3-0357@i+IºÀ9{úLaØÀ:©­
åÀ;vj!
?ññüÌï²U@
sà!"M¥@W=ÿjþ?ïøñ¥8"¿â4z/"bë¿ã$–-º‰¿îL‹Ç§|UNASNonenone?ѤŸ²zÄ­?ÌW¹Äw=?ç-°&ª?ÌW¹Äw=?­ùÕ§
3õ?¸¶#iâA?î b¥\Á?¸¶#iâA?ѯôRŒ™?¶ÂLªÇbá?ç(Ö¹³y?¶ÂLªÇbá?®üK6SB¸? oN'$J²?î;LšËÕ? oN'$J²3FGL J0506.9+0321@h¦$žDúÀ5_â'@·€À:Œý­?hÌÀ;»*VëŸ ¿ùkm´3@Eþw?üމ€Fâ=?ÐaÇnÅ?¸*Ùô,׿ßAׁ[µ¿Ý&ÇojÆóUNASNonenone?ïßôÎòH'?r7ïG?p˜†Û·ˆ?r7ïG!?ïÛþ@–§?|­½Õ/µ?rß´¬x%?|­½Õ/µ?ï1Ž¥Iˆ?ü}ÔFâ?™Î+VÎþ?ü}ÔFà?ïý›KÉP?;8?¦?3ó%¡µƒˆ?;8?š3FGL J0507.5-0906@j)ˆe"¯OÀ;0÷Do›™À:w©"ÉÀ;¹/š!~Ö?2ÏO§°k@S[žnH@ÀÍÆ¿à£ûiº¦¿çˆ¶xU.ä¿åÁȅÑvç¿Ø¹û{ƒPyUNASNonenone?ﴖL£ô(?Œƒv±†y{?'Úl×ö?Œƒv±†y{?ïÕ¨g´@1?€[ÿR,
?u+Ì%ßç-?€[ÿR,?íýèMÅd?¨ÕuSëë?°½'ׄà?¨ÕuSëë?ï~Ÿ@†|ð?'…ÜŒd?,ï0aö?'…ÜŒd3FGL J0512.0-3737@n0mÚÎîÀAˆƒ¡	ÐcÀ:¦í_‹ÎÀ;æ»:Ôe?Ér¤|‰Ð@
u>mÎå@™Kãö	?ïÚÙÔ¶êÒ¿ê+ýw˜œ¿æ
W	.Û¿×L…ϸ9˜UNASNonenone?ïûá¹óE?HÓæ+v?@{¹2îH?HÓæ+v?ï݁¹'O?yãù&qO&?q?#>ðX?yãù&qO&?íñÄB¦€˜?¤ò—S
%?°qÝêËû=?¤ò—S
$?ïl=ªÛ?"$[RÎ?œxJ¿Ä‰?"$[RÏ3FGL J0516.6+1012@hû¼¾bÀ/v(í_ŒÀ:cŒT6¸úÀ;yÇg2>A¿ÒÚ#ޒ®@Àà"ÍR?ÿþî_ċ¶¿ê…³tG`οâÔ¤::¿Û¬³Ì9˜Â¿À4?¤ÓUNASNonenone?ïù¬érõN?M>­"+F?ILZ4*ÇÕ?M>­"+F?ïÎV•ðÀè?…}bb´B?xÔµŸ‹~?…}bb´B?ï©þQE?€Þö<Ý?…¿Àk˜®Þ?€Þö<Ý?ïîÝmÈÍû?\8z"&$¶?a"'72Ó?\8z"&$³3FGL J0517.1+2628c@fSµIùHVÀvvþdŽÀ93PdŒÀ;}#AM¨?އµËYÓ@@ó#x«
@=ô|ô¿âØ(š L3¿çŠK}#cª¿â‡ê©›^/¿ïÿòh´UNASNonenone%?íਪ,x?ºÈÛyºÃ?°úº®œ?Ê?ºÈÛyºÃ?à"•°¼N¹?ҏƒ:°{?ÞÖԞ‡b?ҏƒ:°{?è0p¯?µ"™¥ùGù?Ï?Ž?ùC?µ"™¥ùGù?äôA[Íg?¼"?y©sÁ?ÖÙ}He1?¼"?y©sÁ3FGL J0523.3-2528@l†wFˆzÀ=ӌ†‹ŸÜÀ8£¼:®Q¸À;iÉü7ôc?ðî[Ý÷A•@R$óÅ@;ÿûù5¿â‡¡1h'Ë¿àq•¥ ê¿áUôúâ¿î²"ãøõUNASNonenone?«l¬z""?¯ðÕ[·ÓÚ?îI58]ÖÏ?¯ðÕ[·ÓÚ?­¿_‹Ð±´?¸¾e[]Úõ?î$
Bôä?¸¾e[]Úõ?Èfm/9¶?´Ê·~p‰?éæ\¤´1'?´Ê·~p‰?Ã4Ž=Š´?ªèf½<›=?ë2Üx°T?ªèf½<›<3FGL J0523.7+3328@e´×
=p¤¿÷"'àÙìÀ9;þ®Ç(À;#Ððx?ÁÛøCžu@
E¤—yƒÐ@b †ˆE¿äŒKÑaæ¿éè¸
"'r¿ë3R¼ ¾M¿â"3í~"QUNASNonenone?íp?
ô$?µTô/Ž:Ï?´~¯˜^á?µTô/Ž:Ï?ÞZàAjŸ6?ӇÜgÜ2?àҏßJ°d?ӇÜgÜ2?ëÌüCÐi…?­_lk¶'?ÀÌð¾Yí?­_lk¶'?émðß2Ä?¶ƒ
óRpÒ?ÊH<ƒ4ï´?¶ƒ
óRpÒ3FGL J0524.4+2839@f7…ðoiDÀ.çğסÀ9SS@ï´XÀ;5ÛNoϜ¿ñš%ȼqá@ÌwSH§d@þ[`m~¿ä ñðÞ¿à(çY.ß*¿ÝC—ñ	¿àø®Ž.'¡UNASNonenone?ïês{å?cõ˄¦¬?eŒ"üþ?cõ˄¦±?ïCô>–ÌÁ?ª)Œéo2?—x-&h?ª)Œéo1?ï`ž³Ô?Ž°£RŽ?"ì)…|}a?Ž°£RŽ?ïü\–ÿžÚ??,±h
?=H	1F??,±h
13FGL J0524.5-6937@q"Ë]ÌcñÀ@jq¼Û¾À:VýŸÓo~À;šFfޏ?Öà•©Ay¿@Âԏ‡?ú"YwI8?ïíNc œê¿Ýwúã`¿à(¨dQ}?Ì@´Ê'M	UNASNonenone?ïö…î"©?TX6Á͵?Rô#»Â­H?TX6Á͵?ï閆³t%?sDÑ4ݓŒ?fiyL‹ÚÈ?sDÑ4ݓŒ?ï lؖÔæ?'™;â¤?›òdí%c#?'™;â¥?ïÁAlE?|w^N
Ôa?1_rÉÝû?|w^N
Ô_3FGL J0525.2-6614@qD¾aÏþ°À@¥ÌBcQßÀ:ëíúCþÀ;¤ß³Y^@ÀÊJHùn@ ]-X@Ý<à†(?ïóšÑýä¿ß(l\ìâc¿ãѾÓS¾]¿Óâ'–¶ªUNASNonenone?ïþja=û?mÈNÌÒ¶?/‰Yì Oi?mÈNÌÒ¸?ïï·x":?j'R°‰j]?`H‡áÝő?j'R°‰j]?ïbךò†Z?mBYs?"¥¡¯4¼?mBYs?ïÿð;㬱>è'Ñ-¶öU>߈8¦†´>è'Ñ-¶÷.3FGL J0526.4+2247@fÛü;OagÀ¹¹"á£ôÀ9q—Å"/À:Ç)óë?Ýa`r=Ï@'üÆ>@<wà6a¿ë>ñöZ˜[¿ãô‰»fY7¿ééY³$°¿ÈŒÌ¡Ù¯UNASNonenone?ì 'dæB¿?Á½—'[º?¾ûlØÍê?Á½—'[º?îíïÞÂ:…?°Odìš?¡!ÜW¬?°Odìš?éÞþDnï?¸¼;íö¶?ËЄîDD?¸¼;íö¶?ïƒ馮#?‰=+DéØf?9E–TwJ?‰=+DéØf3FGL J0527.3+6647@b2(õ\@1Ä&5ïÀ:¼ÆŒ@ëƒÀ<Ü<¬X¹?Õð%cß@àà+yU?ý T "žX¿ïy<G׎?è«ûújr¿Ç4A¢D…¿×СõØ<UNASNonenone?ïö#³Ó?Z­†îö?S¹ïؘZK?Z­†îú?ïÁÂìSî?…rÊUš?‰Ör	?…rÊUš?ï‡{³–.N?‡ é
uç;?Ž!tl£?‡ é
uç<?ïiĖՕú?ˆ´¢4«á/?'Çm%M@Ó?ˆ´¢4«á.3FGL J0529.2+3822@eFÕ䣃'@v @hÀ8éæè¹À;+%Â1?ï&gâ.@aÔ=ÚV"@D¡àe¿àH0…PXտ馃('ÄÛ¿êâ3ß´
¿âxC*¥UNASNonenone?ï@àèD#?S7è¸Ð?—ãüÂ÷{É?S7è¸Ï?åGÒõàU?Ól•oÆý?ÕpZ?Uñ?Ól•oÆý?é–í/ìl_?²S,«0?ɤK@NNƒ?²S,«/?äĊ¿Ó±™?½ì¼äx˜W?Övê€XœÏ?½ì¼äx˜X3FGL J0533.2+5944@cõÐúY@,8ðAFmÀ9·´Ï€tÀ;"A® 9?ôw¬NÒöÝ@´¨€èß@¾?–Bø¿Ô:"´`"¿è
‡"¹ ¿ïÿ"[}em¿äüèjÚaUNASNonenone?ì|	á£'?¿m"§0íZ?¼°÷jãò?¿m"§0íY?ê\gIë¸?ÐR
U®?ƎbØS±?ÐR
U­?æÀÝPLÛ?´–Þ«a!?ÒèE_fH?´–Þ«a"?Ï7#3é·w?Á"ºU
â?è273'"?Á"ºU
â3FGL J0533.8-3754@nYcˆe"¯À>âôðØDÐÀ9ñjÉ¢uáÀ;ÇB??°ð¿ø«md¼@4¤m23@¾÷€—:¿Û·çÉ¿é$ {ÿ¿çô•qIw¿Ão¨{×\UNASNonenone?ïû~p<ˆ?F0Jˆ\?B?
ߖO?F0JˆY?ïî@£¬H…?kφJÇR:?a¿\S·zS?kφJÇR;?î¶+Tï]…?›ÅýÔÝ~?¤J±
'´?›ÅýÔÝ~?ïÿ­ º¿ú?¸Q™Aй?—ÑP'F?¸Q™AÑ 3FGL J0535.3-6559@q=Øâe,À@("_õIÀ9ÖÇÉWÍFÀ; dË[³…?¿ti"Ä@Œ!Ûé@˜¾_쥿åèå}C£¿âíɽJÏ¿é¯DI8¶³¿×?°=†/UNASNonenone?ï½ZGË~3?…³ŒkGÌ?€©n
 s5?…³ŒkGÌ?ïٜ.ÖÒ#?€9RV°#?s1蔖îÏ?€9RV°#?î'ÙN«Þ?dP±óE?§ÒkBD?dP±óF?ï'³®ÏÎÖ?M.™¼ê'?›	Š&%)?M.™¼ê'3FGL J0535.7-0617c@j=pdìé£À3¯—Ý÷wÀ9Kd'`˜À:ég¬·ƒ?¯+«ãõ½š@
¾‹Õ‹¸0@+Þßsîd¿ãb¡Õt³~¿çi¨$*¿ëE|Ђ¿ÓÕ¾î'Å?UNASNonenone1?ä¬02°?Ð#(ÆÇ?Ö§Ÿ›ÏüŸ?Ð#(ÆÈ?ïUÒÕM?°O
⊜?œE¥V^$?°O
⊜?èÖLU•¨?·mvµC$Ú?̦Ϣ©©b?·mvµC$Ú?íòñß«Ã?¤©kF²B?°oÈq¡ð?¤©kF²B3FGL J0536.4-3347@mÉ{Ç÷zöÀ=o¼¡ŸÀ8¥»^æ?eÀ;‰al+¢E?ïÔ$
6°|@5"×ëŽÚ@WQ­Dq¿åøó	*(Ñ¿åù?®/—Œ¿âîü"þ"Þ¿Ò¦°UëUNASNonenone@?ïÿÀç[æ!>ý½ÙÀ*êÞ>ÿŒRï þ>ý½ÙÀ*ì
?ïéú0N`R?peP¶kÁ™?fϱŸ­ò?peP¶kÁš?–t¬?…‰5€uMô?‰ÚbùU,?…‰5€uMï?ïò÷ú¥U?Vg.È]PÒ?Zà
µUõ?Vg.È]PÔ3FGL J0537.0-7113@qŸIšé$òÀ?ŠµÃ›Ë£À:'q^-À;'lSq?ׄð4m@/ÒxÞ8@Ü )€­¿×
ú7œ¬ý¿ë³»õÔ¿êΚr1 ·?¶:,µÎU#UNASNonenone?ïåÂS•Ç?sJÓ£A,?jñ=¬j8ñ?sJÓ£A+?ïçWžl0ž?v¬^·[ð?h¨a"Ïcj?v¬^·[ð?í*[®#?©â©é"?¶­"þê?©â©é'?ï‰UPûC?‹˜ˆ>¢·?ª«Á/?‹?‹˜ˆ>¢·3FGL J0537.4+3604c@e ¼¾aÏÿ@h›_lw"À9ƒÓQKL/À:à«ÁºJ?à ¹ü*@
ÈQÉ÷/w@+ œ'­¿å ¹8ùÏB¿ã³Ó'7X¿êŽJÂ,¿Ý—…Ó>+	UNASNonenone ?ã
Bl튵?ÑâU¹v?(?Ùå{&$ê–?ÑâU¹v?(?àCÊ&Ü/
?Õ\9a_þ?ßxk²G¡í?Õ\9a_þ?åjÔY‡å?ÁfÖÛYCÎ?Õ*WMÌð5?ÁfÖÛYCÎ?Þ$Š¯¢?ÄqÿˌŠ?àí÷x:¨/?ÄqÿˌŠ3FGL J0538.8-0341@iû}¿H€À1Ò=p£×
À9™AÞËÓÀ;2qúï?ò2JˆÎ@ž'‰±Å
@ƒßà›¿Ùb\ik<¿ìWG†ôž¿çq6Аj‹¿ïÿp'|¾UNASNonenone?á¹m$¡D?ÎéœÀú6¶?܍%ö½y?ÎéœÀú6¶?ÀC¬^0?ʅ{vò¥?ëï èsü?ʅ{vò¥?àüöQk?·s€.Z?Þ](æ?·s€.Z?±Mx®/©ó?žî;!¿d?íÖPê:
Ã?žî;!¿d3FGL J0538.9+1646@g³&¿‡iìÀ£¾"åÞÀ:ütðmÀ;t!퐑³?è«ñàØrr@ƒU@m-?þ@^_0çÿ?—µo	¹lg?Ü'§ÂYßοØeo™H™¿âÄz\¬B-UNASNonenone?ï¯Ë´5?†VÂÏè?T?"
?'ÿ²É?†VÂÏè?T?ìˋÉäÛA?ÁeÌU"ÍB?¹£¡°Ù&?ÁeÌU"ÍB?îìÈ­Ñ?•ïǞ(M?¡7"ê?•ïǞ(K?ì}[°Ç}?¥.y^Å?¼"yÇT?¥.y^Ä3FGL J0539.9-7553@qô¢}ŠÀ>–~
ÇÚÀ9ÐľáQ¿À;Â6âëC?²J…^t
±@SIÑ«@š'@‹¶W¿ç¼ŠM²v›¿àÕ6Ó@O¿êÉâ?Xc¿Þ~ØdÒßÙUNASNonenone?îäQç<åZ?¨+`ûúf?¡ºáŒ1ªQ?¨+`ûúf?ï•5ÊÜH?š—Øæ"á?Š»²HîD?š—Øæ"à?íÎ*gUW?¤}ÝÄN??±Ž¬ÅUGy?¤}ÝÄN>?î.΂#?ŸQƒ,Ù<'?­ßÈ&?ŸQƒ,Ù<'3FGL J0540.0+1208@h7‡?úÁÓÀ#¬U!š"{À:
ï°ýcnÀ;iþûôÅ¿÷÷äXÍ@œQþ'@ÛQŸÚÑG¿µf#@9¿ì{
jð—¿ÕF"¶U'¿Ó 'ü¨mÙUNASNonenone?ïþÄÀh©?(. l=ƒ?#¿£ùul?(. l=®?þL¤?›Z­Â§œŒ?Š[Àl×?›Z­Â§œŒ?ïÈ`Ëì?yåQÐzÕ?{÷Oš	ã?yåQÐzÚ?ïÿ×j×L¶>ùSàÖȌ>ôJ"Y¤ó>ùSàÖÇ?3FGL J0540.8+3503c@eÈ}¿H€@Þì9yžRÀ9QؗÜ*8À:Ց¡}"ª?×týý`,T@
ßÈß'·@* À){N¿¨Q¾N.â¿ë‹Sß¹¿èҘ–dZó¿á+k4›,UNASNonenone0?è$Œ¹df®?Ì݉²Öâ?ÏmÍneF?Ì݉²Öâ?ëHt&N?Ç ˆ1Ùò?ÂÞ/fÅË°?Ç ˆ1Ùò?æ0B>2‰?Â
ʁ{¯Þ?ӟß{ƒšî?Â
ʁ{¯Þ?ëçVf•Â?¯`€"Hë?Àcæ¦e¨ú?¯`€"Hê3FGL J0544.7+2239@g(-¡"ú×À"ôß:›À9m"š\7À:Ȫ-e"Ù?Ë%Ì~"{‹@ûäêû¶ð@ýÖàL'¿ëd¯N"¿ìiPjjq¿ÐŒ÷£ÿ½Õ¿æÝÎzªsºUNASNonenone?ï²=ËþÇ+?—pwÍ@6Ë?ƒpN5L?—pwÍ@6Ë?ì†XA}ð?ÆnæòVëd?»Í=÷Ä"?ÆnæòVëd?ëçÇc {{?°ÔŽü_Ê?À`âs~?°ÔŽü_Ë?îX S?ªÉºñã?®oª}úÎ=?ªÉºñã3FGL J0546.4+0031c@iœuy(àÊÀ,Q3ß*À9g<kÁ:À;!1ZL?ëj¾ÿs'@Îìt‡ç@@ŒTçÑá¿ÞxoÖ:ñ¿ç–¢ˆƒ¿ìxªô_ãÀ¿Ý)1þûLUNASNonenone ?ëôÊØ9³I?¾;
Д?À,ԟ2ß?¾;
Д?ín}ƒÁâ?ÑS23}?´Œá÷0í?ÑS23}?é˜KÑ>'ú?³Š.©?ɞл¸?³Š.©?çG)A?½`A"?Ñqùý­Ñ?½`A#3FGL J0550.3-4521@o}n—OßÀ=H¤TÞÀ:´ƒ)ìÀ;¤B"ÏÞÀd&Æs@üЉż@C )"¿çbò†ßû¿æÆ'Ûjþ¿ê¸NÉøÃ1¿à"}ÊþcUNASNonenone?ïü[oë^?=‹#‡?=#€¥–?=‹#‡f?ïîÉ:ÜË?m¦ç?¬N@?a6Å#ì5h?m¦ç?¬N<?ïxpÉâ
?ˆlšRk ?üqæþD?ˆlšRkž?ïÿÿÂHû>—S¾'z†Ø>~ó['Šçç>—S¾'z¸"3FGL J0556.2+3933@e~P]¥@7.jwÀ9-—ïunAÀ;_	ðCÊZ?Hږ!\¡@¶†ü#»@¾| aõ>¿æè'Wގ@¿íbääúƿꄉðŒÎ
¿è=¡íêÃrUNASNonenone?ï¾ZYØ?ƒKQ"mC?€i©¸Iç?ƒKQ"mC?îS†ûâ?¿+fu×2?®gêǐAã?¿+fu×3?í†ìÛÃs¬?¤épŸf?³È™!äbž?¤épŸf?íMJ»{?§.àö¹?·5•ª$'=?§.àö¹3FGL J0557.7-0720@j®›¥ãSøÀ.}Ñ¢£YÀ:->9 ²þÀ;oX)ŒÁD¿ðä/,=u¬@ü‡ÝÚf=@/;ßÕA¿éâ¼"ä;¿Ó õjÈS¿çà´¡ÃðÁ¿ÆçãUNASNonenone?ïÕ{BxO>?u2=³pÍF?uB^ÃØ`ç?u2=³pÍF?ïÑu;r–?ƒ¿Üø{?wEtbFµY?ƒ¿Üø|?î–~²¤s?—j)"«Yÿ?¦˜Õ¸Ó?—j)"«Z?ïùg54ד?I˜¬³r''?Jc+,¡³‰?I˜¬³r'‹3FGL J0559.8+3042@f!ê5"`@~½à ¿(À:+0/r´À;pê‹út¦?æjÞu–°@
N½u@ô½?û`zßDH¯¿ïÿö(výÊ?ïþ`  =Ú?cÝåÉQÿ¿Þù…ét´nUNASNonenone?ïÝ+ò>¹¼?mþ®"ù¸D?qjà£!F?mþ®"ù¸D?î‡ÝÜÆ«?¶Lµ¨é†Û?§'">c•R?¶Lµ¨é†Û?ïJ'cÐs¼?ŒðÀý,¯]?–¯³…ñˆ…?ŒðÀý,¯\?íµh\#?¬F¯³å?²W¤½Nå?¬F¯³å3FGL J0600.4-1934@l-1;â.^À3¼˜å>³šÀ9âÆo»y¾À;­1"́þ?ãٍ«d@®Ðǃ@r @§ºï¿è~u΅«ó¿é5Íí3J¿è&s†¬ÏN¿ïÿHÔ|¥UNASNonenone?ï~$0q7?–²>ü¶_?;yîQÙ?–²>ü¶`?â8<‹%jì?РñB&õ?ۏ†éµ*)?РñB&õ?íTÆ!^!?¥L†‰C™?µYÎ÷åþ?¥L†‰C˜?ß·d-¥ÿ…?·Øn\@ô?à$Mé-=?·Øn\@ô3FGL J0601.5+2309@gYW)²€ñ?ÂÀË6ʗhÀ9N˜0
À:íÒä>š?ÛËÆe!@—ñ5·ÇØ@àšüI½¿å²y3‰æ¿åKt­¸¿éc™Z¸¿ç€ †eéUNASNonenone?èÁea'ê?É.]·?è|?ÌúkþyôT?É.]·?è|?ÖÕ®ÂuÍ?ÒÏöo¶Ë?ä•(žþÅ?ÒÏöo¶Ë?ç"úâhP?Àf<ªGA?ÐÖ
;/Ë`?Àf<ªGA?èdÔӞ/?³û^Ô¼åk?Îo˜¬±‡B?³û^Ô¼åk3FGL J0603.3+2042@g£ùHUÚ'¿æðí=…À:c–j:0}À;.LC¥q?¨âg-¢Ê@	ºRøöKv?÷ÿŠŸUÆ0¿ï|	›ÄC?ïqlÜÍ ¿µ/µz¸½R¿æb"¬
ÔCUNASNonenone?ï〱Ö9?sPíâŒ=?lNî)Ç*?sPíâŒ=?áSø0š?Øìb®2?ÝXŸáòÍ?Øìb®2?î·@ll"^?™¢yùm–I?¤‹ù96Ê?™¢yùm–I?íÙèôßÍ}?´§'M3·?±0¸Y"?´§'M3·3FGL J0605.0-0000@ió(àÉÙÓÀ$š¾'›þÀ9"àê'À;Xƒ°j?Í*™où@—8v,®@'T"¿Ò@C"OÇ¿âR€"ÁÆè¿Þ{>í¼¿ØèÛ8þ׿UNASNonenone?ïèT10̦?jlÍE–Þ?g«ÎÏ3Z?jlÍE–Û?ï2cȉ…?§­jbðµ?™½"†îÏb?§­jbðµ?ïRy`|°?"fKÞÙ¸?•°ÓðnJ?"fKÞÙº?ï¸/"é?q¸¹u?üt¿ç?q¸¹v3FGL J0605.9+2039c@g¯Þ¨—c¿Éß8IÈuûÀ8Àº;А§À:¤®á){?ô¶@K)t@cä¼Î@Þþ€N?ÎR	 pV¿äùóK'£×¿ë%Ʀˎè¿è6­Í>sUNASNonenone ?ž²g'¥ô?¤`ª®öR?ï
lÃrׁ?¤`ª®öR?«hW1üͬ?·^ë3=?îIzŒà3&?·^ë3=?ËÎûzPÕ?·i&p0V?éA!kÊ»?·i&p0U?Æ4üڞ?²2çµÞô?êrÀþÉXy?²2çµÞô3FGL J0608.2-2306@l³­À˜$À3hOô4ãÀ:r(œ×;¼À;áàÈðŸ?àùµI^ª@
úp­½@štŒB¿ä´×Qyß¿ä@¦ñ›ä"¿ÌeÔ
È¿ïÿ£©	pŽUNASNonenone?ìq'Åš?Çå–rŠœ«?¿ŒséÓ+ƒ?Çå–rŠœ«?éqLÌÁÙ¦?Î8vƒL"?Ê:ÌÌø™h?Î8vƒL"?éý9Wln?º'$\W`?È¢NGÃ?º'$\W`?ëKqÁÝ"¥?¸be…6Ä?ÂÒ8ø‹un?¸be…6Ä3FGL J0608.6+5328@d	 {5*"@/›Oe™À:Ʋ˜¬À;œnCªy¼¿ë½ñwÑó¨@áÖÚAÕ@ðºà'$Ö¿µG㈿àŽæ•ÔF¿é¤Î#"¿ã'èd6¿UNASNonenone?îÙb§é^?ªåå(µ5?¢iՏ1j?ªåå(µ4?ï¡'
–Û?™ÞÃ˶?‡¶9üšI*?™ÞÃ˶?ê‹RßÂ?µ‡GkŸêx?ÅÒ·ˆ€÷ß?µ‡GkŸêx?ï¬ç1šm?'Ršgô¿i?"Æ3™}$ü?'Ršgô¿i3FGL J0609.2+2051c@gµzáG®?âÎìóàÀ9-J´O(À:˜}–-ÔO¿ãoXš9Á@
n¹?!@.'`@3¿Ò1#"Øå_¿äÝ÷½l4¿ë°²@jºo¿Úð¼UNASNonenone0?â‰ÑÁ×Jª?Ðó®ÓÜg?Úì\|Qj¬?Ðó®ÓÜg?èk««Ù6?Ò³È*y©?ÎQQP›'ß?Ò³È*y©?äØ0^=?¹¾Œí>?ÖO۟ñC…?¹¾Œí>?ïiʑÅý?"T±x2?'Æ­Ç@_Á?"T±x23FGL J0609.6-2851@mnµÇ͉‹À5/.ÌțÀ:J¥öŸ..À;æ,_Ú[+À"¦ÃMÈ@	A–xQö@ý`O¿èT-ĉ\`¿æZýñAѿ㜒i=u¿ïꆳ&Í8UNASNonenone?ïðTJuö	?l°DJ
?_Wkì®?l°DJ?ïÔló7ì?ƒƒQ;3z?uõI†d
Z?ƒƒQ;3z?îòѪI	­?• öòÐaò? Òå[oe+?• öòÐaò?ïþ¡Éi\ú?0§Ü•Hñ?%ãij0d-?0§Ü•Hÿ3FGL J0609.7-1841@l.ÄÑ¢À1bÑ9C­À9¢aÅíµ{À;›ÀoÇ88?ç	ů)×@~ÛËÃ7x@cËè ¿Ó;ùæ`q°¿å©O°´¿ç"Ky¯n¿æµêpLšUNASNonenone?ï…B«

Ü?u"•O?Ž¯U<¼ˆÿ?u"•O?î¸ÏÃÖxo?¯™øÚgQ?¤s˜y"?¯™øÚgQ?섋Ý¥?®%ÐÀB?»Û§Ùê×?®%ÐÀB?료¾Q·¢?¦²ãZ¿±?Áq͹!v?¦²ãZ¿±3FGL J0611.5+1957@g×.œË}A?丝jßrÀ8Þ$ZR[íÀ:¾Dä5Ÿ?ôjÅ(=¶Å@³ÅPÉ@e@v'®¿ÂtÂvÔêö¿èvssârH¿æˆÅ(
,¡¿éœuʐUNASNonenone?ˆí³éÜ%æ?˜.E›‹ ?ïœI0Xh?˜.E›‹ ?¬Si3É?½0>áÌ«6?î?êÇ)lÄ?½0>áÌ«7?Γ
äë¬?¹EEûºR?è[=FÜ?¹EEûºR?ÂþŸ…¯­×?¨çºÎg?ë@X"Š?¨çºÎg3FGL J0619.4+2242@g¥Ô¿	•«@l'"øÀ8åtË"¾À:dX R…ß¿´j摏¢@Â]](O@ƒ 0w¿æsñœ÷¿àr¼‡Ò".¿ßNr\q¿äI͖ÑOUNASNonenone?ït5S!õZ?.¦‰ó?'yU›ÁTº?.¦‰ó?ï±gxŠ'÷?"	ÍzÏp·?ƒ¦!ÝvL?"	ÍzÏp¶?ìçÝô•#ã?©óoØe	ä?¸Á[Vàç?©óoØe	å?ïžÚ2Ã?ŒÊ<n?ˆ`	sO;ó?ŒÊ<n3FGL J0623.1-4143@o1"…]¢sÀ6ªk\šÀ:…vWu1ÛÀ;âº5"¿ã¥®éjšÜ@©'#Sl9@R?'Kõ¿í^¤blÔ?Ï(²aøª¿äc•åHÞ¿è˜Ò?05UNASNonenone?ï¹5æ­ù?¦ÒŒ®?ŸÙC*@ß?¦ÒŒ­?ð;Š?µ^"/¬ì?¤6øüG[?µ^"/¬ë?í°n¥1´?£%çbÐ,?²$ŠÖrZ?£%çbÐ,?ï#·{?"†ÉŸoy?›œÉŽQ?"†ÉŸoy3FGL J0626.8+1743@hLœàuöý@
eä`gIÀ9;\Í`qÀ:~·îï6"?ôKg<O;§@&X¹Õy@˜Ëßçܞ¿ÛWÈ¿în…(jϤ¿çm+?Úò'¿ÄÒ*Þê aUNASNonenone?Ü®ÒÅ?Ë-½Q¾Û?ᨖr|þ?Ë-½Q¾Û?뾡Ì|4?̋a9²z:?ÁµxÎ1?̋a9²z:?ãap×Iý?µh$Ûq'?Ù=ÎQl?µh$Ûq'?é#Ûä¸ú?Ãf–‡#Ü·?Ëpoù?Ãf–‡#ܸ3FGL J0628.4+2429@g'^_0çÿ@ÔÃ\á'fÀ:û¥þ+êÀ;\nªƪ¿ÛLçDd@
ç݉Þe¦@¨‡Ÿqü¿Ýp_
ô¦¿Óø¬
ÿI¿æ=î"2	¿å‡†UNASNonenone?îóÁbv?¡JWb¶	? Ãî9Þø£?¡JWb¶	?ï¤XzÔ?–¾›Cj	Œ?†éáy>ÊÃ?–¾›Cj	Œ?ì݆۞–ª?ª}òXW'^?¹É#J®?ª}òXW'_?ï¯(9±Bõ?|°m‡ƒ?"5ñ"¯C?|°m‡ƒ3FGL J0630.2-0929c@kaЦv ïÀ!öúaZëÀ9¤,ŽÔCºÀ;5,)Bï?ò>»Õ-Ä^@!\q@ñgya¿k²ú•gC¿ìÒ
}¡/T¿âu	u…ÏI¿ïÿ'?¼UNASNonenone ?ä¦TóµôÕ?Ëjn;6Z?Ö³V"W?Ëjn;6Y?ÒÙ«ÿ-¾?ÑkE|nJ=?æ"*i|!?ÑkE|nJ>?à58¾EŒ?·™vZ'Ð?ߕúƒtç?·™vZ'Ñ?Ò7¢ŽˆZ?¶½9ʙЋ?æä.¸ô»Ó?¶½9ʙЊ3FGL J0636.7+7115@añ~|áœ@8mDþ6Ò$À:
{À;ÑïSàQå¿øwƒ…*L@Ùº÷7Y‰@ڊ ,…Å¿êûRAsñG¿äNnU>¿ãš'"¼²p¿èèÎ̶IUNASNonenone?ïÿNä%³
?"»'~*™8?#{Ižg»?"»'~*™Y?ïÛÓ§—…?|Õ©Ä*3?r,w4<Ì?|Õ©Ä*/?ï´7Vb?…'®²R?'ò*|9'b?…'®²P?ïÿ"Fž? ì¼À<¥?_{·,J3? ì¼À<Ø3FGL J0638.4+5704@cÍ|ßýa@4ϋ&9O­À:Á=L'©À;íó?']<?Ö䟫›=¢@}'ûr|Ÿ@jÎ]=s¿ìN^·'ËA¿éÙQ®¯'¿Ë	àØ·*"¿ëH©2øUNASNonenone?ïþ_ FÖ?3†7>çZ?*
ÿû'•|?3†7>çL?卑JŽ?ÝjŠˆd?…ú­zÜr?ÝjŠˆd?ï"à+¿ð?‰Ä©Ï5+^?ŠÇÛõ?‰Ä©Ï5+]?ïyKÍù‡?ŠðûÄ?Ö†_ Ï0?ŠðûÄ3FGL J0639.9+3250@fÁª:э&@(9äSÒÀ:
¬í#À;ˆðÔéÒÀw4x­Ç@6 \@ó@*·àŠ"¿ãÊ´p×ÐÙ¿æÍó3F‡¿é‡¤t>d¿ãžnÖRªUNASNonenone?ïùMî"?d?L.P¾4£}?JÈEïpÐ?L.P¾4£€?ïãÙe²Ö1?xbK:{®Ë?l&šM)ÎÔ?xbK:{®Ì?ïg'ûÙå?Œ7ˆ`tÛq?" "ÃT?Œ7ˆ`tÛr?ïÿßÛ`Ûe>û7þÆOò>ðO'M-¥>û7þÆPË3FGL J0644.6+6035@ca…H©¼ý@6˜)à¤&À9¬Â7G"êÀ;߁SQ¶¬?­e±p›@eyþ§@63Ÿi½3¿ê…wßƶ¿à­¦t|¿àƒ¥p´À¿ÝŸôôÖx•UNASNonenone?ïê]×;^?|–ðÞÃD?e¢(Ä¡êì?|–ðÞÃE?ïÄj+`KÓ?'ÑfÓc'ÿ?}ÊêOÚ6?'ÑfÓc'ÿ?ïA§›»ñ[?"×͵¥?—ËˆÔ¢?"×͵¦?*_9?|+íõííw?‡Üu|(1¢?|+íõíí{3FGL J0647.6+0032@j€Îš,f¿ã"‰ÝŽæãÀ8›èPðÀ:ñ#±µð?ì­½Dõþ@.{ÏÚm@¨Ã ©-`¿ÚPâǜ'¿ê½"6± ¿çߕÒ9É¿âVxÄPÁ'UNASNonenone?ê6Š€Œø¥?ÃÜô%¢O?Ç%ÕýÌm?ÃÜô%¢O?É%›ô'X?ÌÃÖàG?鶙Û})?ÌÃÖàH?ä™ÄuŠº?¼ñĬ9e4?ÖÌwê‹Ð?¼ñĬ9e4?ßßø'þ?¸îfY=ú4?àÀ>÷?¸îfY=ú43FGL J0647.8+1751@h'çÀn¹@˜Ôw¼À9Ži°ÂÀ;3è?ïÚ?óàÆ>hE@
»þ5¥~T@Ÿ\"¿ã†3é!ӿ죃äY9¿Ý<è7'¿äà劫6œUNASNonenone?ìÅ0§Uj¼?¹?8†Û?¹ÖzÅTª#?¹?8†Û?ëw¡Ž(uR?Ì5Î;ê[¬?Â!yÇ^*¸?Ì5Î;ê[¬?ç÷™<ʙ?²…\]xêÜ?Ð͆jÍÙ?²…\]xêÜ?ÛyQLSc?À֞š©_Þ?âCWYÖpÏ?À֞š©_Þ3FGL J0650.9+6524@bĆnCª@8s¸<òϖÀ:+gÔûoxÀ<µ¬õ–ðÀÛ²t†å@Ó,8Ã@R`E:¿ê£É²ªÑi¿ãd1_ô\^¿ãƒš"ÉÙ±¿ìH¹IY²›UNASNonenone?ïYRû<Z?œ	½0,9?"Õ¼`˜tã?œ	½0,8?ïÚ
Í%my?}¡rêqŒS?rùmICá?}¡rêqŒS?î.¦LqÏ? =¾=*\?­›>hã
? =¾=*\?ïÿ­¦-ì?ó1Ñ+Y?–t"ü%+?ó1Ñ+G3FGL J0657.6-4701@p
:æ…ÛÀ2|?>pÎÀ:`%wˆÍ™À;µ£@âH_?äɝ¶gcD@
!¨[Ô<-@ÄÌ>?î3¦p¿áù¬_ç>¿Æxä ªV¿ê
%Á8L«UNASNonenone?î—a»K?²G?ðå?®v‰äN{X?²G?ðå?î)Gá›M¶?¸O#T?­kæK$'?¸O#T?ëñÖiø?±-kª¥÷z?÷ä8¦X$?±-kª¥÷z?í83†æìØ?ªÂU°ž?¶>cÈșC?ªÂU°ž3FGL J0658.8+2318@hÈÞ*Ã"@'äË:%•¼À:`e)O…À;¾eÌ³mÀtóL¾J@lõvº@ZË`6¿è‹á··ß!¿çOY ˜&¿å©MIg…©¿°ã€("lUNASNonenone?ïô_•‹?ZfE´>¹ø?WAÉîÔçå?ZfE´>¹ø?ïãòŠP"Ï?x/Ù?³?l
u¯{1Q?x/Ù?´?ï4™kY\?•Mþù?ylҔÔq?•Mþø?ïÿáiÿdÁ>õÞ‡b߆>î–›?¶7>õÞ‡bßÃ3FGL J0659.2-0439c@k>§æšÔ¿ÙWŒc¦¬À9-QîÊNÀ:ÙàU?Íu?ÖZãü>Ty@
Ïd9:‰>@3ÛËÍH¿å¯ÀCkSz¿åЬçef¿ägX6Lî¿çf.:ÙxUNASNonenone!?åvâ`^?Ї›Þqé¬?ÔýÖ;?F?Ї›Þqé¬?Ö­^ûô
?Ó=¡GñÝ?ä©P'¿{?Ó=¡GñÞ?è~àr[?»‡€÷B?ς~6"¦?»‡€÷B?é¢ÇUm-?³‰½TvT?ÉtâªKKî?³‰½TvT	3FGL J0700.6+3557@f™³=¯ø@1C'·þ	À:NGKîëÜÀ;Úa¶Ô=?åß*¯ø>@ÖшsW@9¾ Œ'u¿åˆ=^¸ÐŸ¿Ý°… à­!¿êð
-ð¿ïÿOÇF.UNASNonenone?ãӁ?r?ÐPQô1H?ÙÎXýہ?ÐPQô1H?ÖëDª"J?҃_?äŠ]ª¶\?҃_?æ(C@tbÍ?¼mW±Né?Ó¯y:e?¼mW±Nè?ËnÄÏ[s?±tüC?é$NúL)#?±tüC3FGL J0704.3-4828@p-xÔýó¶À1ô®…¹èÄÀ:áH2ŸÀ;Á™úèi¿ÐàF9Ó5@
¸ƒ«R?ÿ–Ÿ‹Á?äß5eù•>?Š9¼Ç?ÐƖ4èȉ¿éåH3ûUNASNonenone?ï3×'|R¡?¡%Š:h;Œ?™…u«ð?¡%Š:h;Œ?î–l·(I?¹zԉÖe&?¦™4†ý{n?¹zԉÖe%?ì¡-§Æq?¯[ÞU†`)?¿âö'ÁÌs?¯[ÞU†`)?ï¿gŠ7¬*?SÛLI?€&rõ"?SÛLI3FGL J0705.7-0006@jÕQ—¢H•@	Â?«ºÀ9ñ½V7D:À;Z³˜H`Â?êN¤d'•ˆ@ÛÛÐö¨@/² %ÏÈ?뗩Ás¿á0DZb–¬¿å·TѤ´¿ïÿ÷ç­£½UNASNonenone?éÚåL$+?Ȏ}úʬÅ?ȔjÏoS?Ȏ}úʬÅ?ä©ðŽ(s?ÑÎ%"ù"?Ö¬ã¯û?ÑÎ%"ù"?âênÇ(#þ?·mÞ©ŒØ?Ú+"q¯¸?·mÞ©Œ×?åƒÞÞ¾?¶­^BJÞ»?ÕÊøCÎBƒ?¶­^BJÞº3FGL J0707.5-3111@nVúñ€À%V"uÀ9Ïi,êCÖÀ;"ëžI+ÃÀ‡¹-2¾@Z±ƒED@±ù`~šæ¿ækMÿm'¿é|áp®úæ¿ç«Ø)2…¿Ú•2c¡ÝWUNASNonenone	?ï߸€"B¦?rŸ‹$ry?p#¿½Þ¬¼?rŸ‹$ryž?ïÇé·}

?CMôÃ?|$Azú×?CMôÂ?îêh"°?•ÎNý¥€§?¡YvÎDÿØ?•ÎNý¥€§?ïÿÿÒá&>•5›¥2#>vólÞÝ>•5›¥§3FGL J0707.7-1035c@l|"µÜÆ¿óñ'©"áÀ9/%Ž/LÀ:žYò»?í†ý1é@ÚHtñp@ôCÀI0Ë?èÞKb©î¿çÐgõ¿êû\˜1e¿éª{"œ UNASNonenone ?Ææž`€è?ǟem¦°ý?êF}gßÇ?ǟem¦°ý?ÑôG‹í?ÏÄØ?çqÜ@:
?ÏÄØ?Õ7áNÅQ®?¼:Ñ|èîO?ådXW)?¼:Ñ|èîO?Ûðh±äé?Áp|C?ø'?ât‡Ë§
‹?Áp|C?ø'3FGL J0708.7+1747@hÙm›äÍu@'y»à~íÀ:d«Ï&CaÀ;·'ä™r,Àï a^ë@ÖúM8—÷?ýc8¢gI¿êD0¦2{ ¿è
¾Äî©c¿Èú‰ÏÞ5f¿¯P8ï—ÚUNASNonenone?ïÿŒš÷Ñ?|ÈOB$Š?ûYBîä?|ÈOB$T?ïäzÚþ?xa;F‰?k…%÷üN?xa;F‰?ïçüaEÃ?nþ~ðGùê?h垺= ?nþ~ðGùè?ïÿý¢xgª>ÀûÁ¦þ/>²ì<«Sg>ÀûÁ¦þ3r3FGL J0712.2-3806@o0¼¾aÏÿÀ)0HZåÀ9ÚÊ÷àÀ;uÕ`EK?êUVß	æ3@Oþáqõf@5SÀqt·¿äÆ1ò/K·¿äŠ‹ÅN0î¿åƒ¾`£Xà¿ïÿȏGÓvUNASNonenone?îuh±RÊ?±KlÏ$Õî?¨©tïúÓ[?±KlÏ$Õî?ézCG¤¨G?ɾŸ¯Ø?Êòám^â?ɾŸ¯Ø?èöYñçé?´dà¸Êž?Ì&›¬8`Z?´dà¸ÊŸ?å?a{!ß5?²}yˆ^ñ-?Ձ=	¼A˜?²}yˆ^ñ-3FGL J0714.7-3924@o^ {5À)dBÇû¬´À9æxT¥sÂÀ;e?åë€@
}ŸVœïº@œÀ? ª¿Ç/I=O…"¿èšÿ'_I¿ì¶yš†åž?Ê•—R+UNASNonenone?ì‰Ú•Ö?¼Uuá'¯ž?»±/G‹QN?¼Uuá'¯ž?ïgÀkƒ?©¬,	'1Ã?"òŸÞ?©¬,	'1Ã?ê>å]ÀË?³1õö¿ý?ÇðjˆüÕ?³1õö¿ý?î\%ê¸Ýó?ªt?(ƒ¤?ª=¡Tr Û?ªt?(ƒ¤3FGL J0716.0-4525@p
quŽÀ-âÏ d#–À:G8£µ|À;Á'²D‹JÀòõ¼Û5@
'1µY¾@åÔܑ¿ì;lÁnþ¿â2öà´¿åM‹\¦/e¿Ý"ÙgK#üUNASNonenone?ïêƒi?hw¸`3ð?e|ÿ–úø§?hw¸`3ð?ïÙ
,¨þG?°ðL\Ù¡?sz髀Üy?°ðL\Ù£?Â@ä?&p!Îb?§UÛÿq²?&p!Îb?ïÿð°nÍô>í™pMý—w>ޟ"dÆÓ>í™pMý—'3FGL J0718.9-5004@pUS÷ÎÙÀ0Vy_goÀ:¦ý/À;¡0-Å5)?ÈN‡Jj:@q¯åC;@"FÀXË¿äbîpFË'¿æeÔñ–¿Ü~;)vÆÜ¿íÊö´Ò°UNASNonenone?ìÍô 7r¾?¹ÕEÐ"?¹ZþDj	?¹ÕEÐ"?çÐ|¬…a`?Ï"¼ct-á?Ð_¦õ=A?Ï"¼ct-â?ì}Mj¡¿`?«üøD&?¼"ªò?«üøD&?éT´3ƒó+?·žjù¨8"?Ê­/1ð3U?·žjù¨8"3FGL J0721.5-0221@kOuŽ!–S@c)ÞÛhÀ:Pc–¨M'À;YeΑÀ¼Š`Á‹Ñ@
›ÔeÈ[Ï@w í?é¶æà/'N¿Ü.Êz¯k
¿áÜu‡t0²¿Øú•aˆºUNASNonenone?ï÷..Íôº?OëÂ<Â~Ø?Q£¢dŠ¢?OëÂ<Â~×?ïφbj–Ë?0h†‹?x<ÎÊ´›0?0h†‹?ïG™HÞÉÝ?ß€ïב&?—Öä&ÄG?ß€ïב(?ïÿƳ¥'É?q;³>gh>ü¦-7u¶?q;³>g"3FGL J0722.2-2648@n9XbNÀˈ¡ú'+À9œÝÖ³ÖÀ;R¡w´l"¿ðóaHDg@
ˆÝrâJ¸@œÁ¿êPGÕpy)¿àՎL"¿å!ÙJåÀ¿ëÊ}^œåÌUNASNonenone	?äŒZìKR?ÉPG@¼
b?ÖçãJ'i\?ÉPG@¼
b?î#6ûxú}?ºBˆ+ ƒ?­ÌHpX:?ºBˆ+ ƒ?èa~€8hL?²AE.vê?Îzÿ^Ó?²AE.vê?ï˯§Ó—?zèT›wi˜?z(,7–5 ?zèT›wi˜3FGL J0725.4-5007@p\å@ÌxêÀ.ɶ'!%À:¼šTª|@À;ØúËÙ,?í+žMÒ@x³yi£]?ÿ€@W3¿á,s©£…‰¿ïÿ·¯'C?ïûûU˜°2¿Þ«úõ—UNASNonenone?ïáħ7šE?t4ÊJ&¿ú?n;XÈe»°?t4ÊJ&¿ú?ïzåúf'?¬­4@ ÿû?£]€³-å?¬­4@ ÿü?îYÕHJj?œÿ¿™µQ?ªb«{Y_Ü?œÿ¿™µO?ïZ±Í‰$q?±µv[ù?"©ÆNÛqù?±µv[ù3FGL J0725.7-0550@kÂW§†Â'@ªÄ°ž™À:&¸©õÀ;']<9A?çâÉ|œnò@äJ¾À¶?ý›ù?ò^W?êIHQŽ¤.?¢U'Õ«~¿¼Rk¡}'¿à)êÚ©Ú/UNASNonenone?ïՉT¾q ?xRÌï¾Û?u;U Ç0T?xRÌï¾Û?ïk¸6ʑ?¥
§?ܘ?'ˆüY&­Õ?¥
§?ܘ?ï+ó¢H?ýݜ\;?š‹¿öÿ?ýݜ\9?îâìY!¼]?"õõ;ˆo?¡Ñ:mä:'?"õõ;ˆp3FGL J0725.8-3532@o`—ÌÀ"ôù;À À:zÑWv	À;qªt³0D?Ðx+úé@"9náŠ@ÞL€S¿éø$ÆLÄÄ¿æ7BÙ»À¿ãõr
É¿½céL&/UNASNonenone?ïÎÜ
.+Œ?…®ÕhÂ?x'úèê:?…®ÕhÃ?î[šUKS/?¹ûÅðÕX¦?ªFZ«JÍ?¹ûÅðÕX¥?ï:™`Ç?"{éè‰\V?Ÿ^8¬Óç(?"{éè‰\T?îòå'[?—к'zmB? Ñ®êH?—к'zmC3FGL J0725.8+0212@jÜÇ÷zö@@!U0H'ÄÀ9|DeNÀ;{àdYEì?Ä<fõÌ@õ½ê0àÉ@zDßØî¿å]àÛÍq¿â7ä¬M·¿âò|Ԛ¿ß8ÅJfUNASNonenone?ï﹌Gú?_zâ¾Âº?`Fås¸	?_zâ¾Â¿?ï˜RŠ_P?˜Xó%Jëã?‰ë]X¨+î?˜Xó%Jëã?ï ™˜‹¨ç?•fDL—…?›ìÌîŠã?•fDL—…?ïX®À£ìú?ƒh †Ò§©?"ê'ë'`­?ƒh †Ò§©3FGL J0731.7-1914c@mRd"¿Æ·\"?ÅéÀ9©ÌíƒüÀ:ì±+†–ˆ?í{‡¬ ÷ @Ȭêˆõ@+ÿwD¿â%q/(rÌ¿í_ÇÑÃà¿ãöÛ¯yç¿×g£àeUNASNonenone!?ì«œi?¾OÍ</™?º§»L·q?¾OÍ</™?ÜU×c´'?ÔcRBîC?áôÕN%¾?ÔcRBîC?èBT+Ë-?¶¹Odƒ›?Îö¯PӃN?¶¹Odƒ›?è¡Ô)®¡?¸Î"¹V?Íx¯YEyü?¸Î"¹V 3FGL J0731.8-3010@n†!ê5"À˜¬}¡ìNÀ:|"}ÙI³À;ÛeìÃã¿Ö•´2Þ4å@ÆËG;¨Î?úµ1 6ç¿ïÿ(Ÿ˜??ïÿ#üY¾¿ÚÒÁb$Q2?ÇñÎ?yδUNASNonenone?ïýªsH…?4Ù¨¥M¦?2¬e»Þ}?4Ù¨¥M‹?ï,Ãßo `?®rɁ	Ä°?šg"ô?®rɁ	Ä°?ïµrEåº?|8·Rn?'£n†'yÂ?|8·Ro?ïö	"gáª?TÌgÓΊX?Sì×0<«¼?TÌgÓΊV3FGL J0733.3+5904@c¿")³ú@<O…ô¡'À9ûçéóNÀ;ùŸ¸—‹¢?¹Q¥mü÷@=X´ÌûÇ@>2ÿ±¦¿ê
π8ï¿ë†ØÕÕÆ,¿Ó½ïù'j»¿èúÖ0´åUNASNonenone?ïÿÝHÔ¼€>ó]å÷kY>ñ[•¡¿¼
>ó]å÷kZ'?ïÈY‡+±Ï?ƒ©qÓv²'?{Ó<j'ƒ?ƒ©qÓv²'?ïâSý´å>?u7Ók,Ûû?m¬KÁ+?u7Ók,Ûû?ïäÿïC?b·† ž»u?kèo½h?b·† ž»x3FGL J0737.8-8245@rq3|™®'À9t_ZÙjjÀ:
jÿR[À;§£@âH_¿ü5V¹u,'@
Üme35Œ?þµˆ€»®¿Ì4Xþ…Þ¿æ×(Œ¼¿Òð[Ç빿Åkí4²uoUNASNonenone?ïþE¹~à*?-ÎtUœI?+¤hýVì?-ÎtUœH?ïèÔèŠ?sS'\hÏ?g+äüuÓ?sS'\hÏ?ï´.¯®ò)?gMܵ?'ôTCuð?gMܶ?ïÿéá7P>í¾ã"{µ>æñȯüÈ>í¾ã"{Ö3FGL J0739.8+1312@iÊsÕº²@0Ÿ(bõ˜žÀ:+ÈbÚÀ«À;µ¢4rÎ?ôT&£,ëF@¶½[À›@àpÍ¥»¿ãGÀ-#œ	¿é+œÔóž¿ïÿÁÄ[D¿á<ƒbê·UNASNonenone?îÐÖu0âQ?«DËÐñ±?¢ò˜¬ñÚô?«DËÐñ±?ékÔLã?҆ªèÇÁ?ÊP¯þπs?҆ªèÇÁ?è²GãOæé?²êäã3•?Í6àrÀd[?²êäã3•?ĘÙÓ¶?ÀôkÍvÚ?êÙɋ?yÓ?ÀôkÍvÚ3FGL J0740.6-5230@p'DЩ*À,…æÿ}úÀ9ՓW`9&À;k¶1€¿ù‹·Shݺ@õÔȧÏ@×ß?k$ç¿èÄéeM¦k¿ßÙØ
e,¿æÊ^Eäv¿ØŠ—È<UNASNonenone?ï‹JTž"d?Ž%û/éál?-jØ^æê?Ž%û/éák?ïÑúÿ"¨Ü?ƒ·:ÖO?w€6+'?ƒ·:ÖO?îJ¥ái©X?œ\œº?«U¡éej{?œ\œº?ïýb75?<hžÑ?7ó|îFV?<hžå3FGL J0742.7-3110@nÆw[0À®S<½öpÀ9{lØÀ;Ød°ƒÁÀ0tY™#}@¯h¸Ñ@½üÂØØ¿à±s39¤x¿èê|ã!ð7¿ä¥ïÑ3º¿íŒì"Š³oUNASNonenone?éÂdÔzÕ?Â{Ô?Èöl®«í?Â{Ô?ïÿïzå?°ê™ðg¨?œ]@£J?°ê™ðg¨?æÞO"ä"?µc˜Æ3?ÒCaº7Òø?µc˜Æ3?ïý¢Íd™¤?Cνzî®Â?2é"Û2Þ£?Cνz3FGL J0744.3+1715@i\í(Œç@3?¿¤Æ†À:0áþ99À;¼RÀ—4e?ìÝ$ݞÅí@šö†M@ៗµi¿ÓÝz:iïn¿âkዲ¿ê—Ž$"¿çAê%DªUNASNonenone?áqAxœˆ®?ÐÜó¢BÒÔ?Ý}Æî¤?ÐÜó¢BÒÔ?â‰òwðE*?Ôóh">ç?Úìu­?Ôóh">ç?ækÎ[	'÷?º(Çfâx?Ó(cIìÚ?º(Çfâx?ÃRtìì®+?²ÿg&2?ë+bÄÄÔu?²ÿg&23FGL J0746.4-0225@k¯\(õÃ@&*¯È°À9¦´%6nÀ;'ø
h9¿Ç*G@C¬@]XXܐ@Eß³.k¿ã¦H®¼ä¿Þý´7÷àn¿àjê.÷(¿Ôá)E\UNASNonenone?ïû§ۘ?Aw1źªÍ?AcÃБŸÉ?Aw1źªÒ?ïÓò}]f€?ID¤R@°?vÁQL¿Ö?ID¤R@°?ï°û`œ?'_ü½ú?ƒÁ:çùØï?'_ü½ú?ïìz²yÆG?Xç @!¤ ?c…M†9¹s?Xç @!¤(3FGL J0747.4-0734@lF`ªdÂø@!£Ð|"µÝÀ9û™
þ`ÄÀ;wÖ	Œp¼?Ùý%	NÞ@fñ/
@笿'%¿ì+£3:Ê?©¸Á"bçº¿à›ƒ†²·"¿åë!²¾iïUNASNonenone?ïρ ÐhR?y>-Òý¨?x?o—ËÖî?y>-Òý¨?í0ô™'ò?¿Y¿ ³*é?¶x[7ÆÀq?¿Y¿ ³*ê?ïT}4Â4?ŒwcfŒð?•oÐYg¹p?ŒwcfŒò?ê?žÖ8Ù?±Dnj­¼?Çï"§ ?±Dnj­¼3FGL J0747.5-4927@plçl‹C–À'ÎÛ0sÀ9ÛS¸
øçÀ;k(zrŒå¿Ð=tÄfæƒ@
pó'ß@B@0þ'î¿ç$
Ù©Ì¿ènè\ ¿ÓÞ d×ú¿Ý¨-óòðUNASNonenone?ïù'›ý*Z?QHE7"?IõV™¯?QHE7?ï¸hq–?‰ê%0šÚB?åã»zª?‰ê%0šÚB?ïÌí™pI?Œ!¦ÛßÍ?bLÑöø?Œ!¦ÛßÌ?ïã ]à:?b'}Em'?l_¢ðÅÉ?b'}Em3FGL J0748.7-5116@pˆ¥ÃÞç'À)1!îgQHÀ9Ê´øš°ñÀ;cÛêw¿¿áiô/3Á›@
ìŸÊ5BØ@÷L_ª	©¿Ù²öcm^¿ïs5Hم?ԡȕc1±¿æÇ"µ¦Y_UNASNonenone?ïüZèXD?AžÒZã?=/ ½=ç?AžÒZâ?ïɚïZUw?†rý9Œ?{2ˆRÕD¬?†rý9?îêK^¿
;?–LüÊ]RÚ?¡[J\J?–LüÊ]RÚ?ïûÏÃue?TJYÉP
­?@Àò)Šhà?TJYÉP
§3FGL J0748.8-2208@máî¢
?ý¸Ž¼ÆÅLÀ9z
>GclÀ;0¿ö$µ¿ÜÞQêƒl@
q†,ÕK!@ìÝÀ$5¿è»q§{ô1¿é
!þÑ$¿Ø'ç5¦"¿ç†Ú6(UNASNonenone?ïð)¸_?d°³Ô5C?_Ó­àA?d°³Ô5B?íº?Á¤"ŠV@?²/OÀŠÓ?Á¤"ŠV@?îJ¹Ð £? m–‡¿-Â?«TbýõÎH? m–‡¿-Ã?ï¼M….{Û?|\Ö7;?€ìž´a	Z?|\Ö7;3FGL J0749.0+4459@eÇ;÷'j@<ž†"ÄPÀ9áÀ¾¡ßÀ;âïÙAOV¿æ ž†~@KÃ Ô ~@ùY_í¦a¿æîÜü'.¹¿â^Ø܋ÂÓ¿â&(¦I€¿ëBýùóÿõUNASNonenone?ïá›QÁëä?n×àJƒ?nd®>ã?n×àJ€?ïÌŸ'p?ªbZ1*6?yø°lGùd?ªbZ1*6?îܐJNF?˜ñø Nß?¢>fû[¦?˜ñø NÞ?ïòÿ÷NCF?VŽŸ¥Ä?Zcytv?VŽŸ¥Å3FGL J0749.5+1320@iç×Ûôˆ@2Ññ{ؾsÀ9ñªÖÿµÀ;Ÿ»@³Nw?éÀž‡§ @ºd>@þ–Ÿ¿"•¿í¿úÙ{?¢Þ,1¿æãtS¹æk¿èfžàs¯UNASNonenone?êhü!?Ã[Å¡'
?ÇÞ\Çã}?Ã[Å¡'
?ëÿ¨pzÄ?Ág;¸±«?À^>ñ?Ág;¸±«?ê†:¬Ïƒ?²e2y,'?ÅçLÁóÍ?²e2y,'?âge<¤?¹àéÔûÜ¡?Û1ï5dž¹?¹àéÔûÜ¡3FGL J0751.7-2944@n½ºˆ&ª¿÷‹?cÃÀ9u°}á­/À;Ù|¸[¿Í_:û ¾@¦H<Ú¦Õ@šÿà iB¿ÚÎmÝdZÚ¿énÞov¿ïÿç
)"f?ïþ¹ç܌UNASNonenone?ïԔª&=µ?†,²U•‡Ü?uµªìá%*?†,²U•‡Ü?í"Æ Ñ«?ÅÉæÚmÈ?¶éÊùwº¦?ÅÉæÚmÇ?ì~¯î1?«­hç´üZ?¼
€Ÿæv?«­hç´üZ?ïýÑb¤1?@*j·QÖ?1wLêÞ~û?@*j·QÓ3FGL J0752.6-1629@mSýÉÄڐ@ôë?{@À9ÍRÿ" À;~%AØèd?ÝâDæ@
꟏&y@˜ÿ•!¿æÜ3"yl¿Ú ÎçG¿âm¡UrÅ¿çj;Çù ¸UNASNonenone?îs6,V'N?¬ÏJUÓa?¨Ì:—Û"?¬ÏJUÓb?ìh´Î«;?Ä5ƒÌÀO‹?¼¿ÊYŠ¦!?Ä5ƒÌÀO‹?î7Û	€?œ)´ê/?¦üŽÂOgþ?œ)´ê/?èñ#º…H°?°Ô¯¹"û?Ì;qêÝ=?°Ô¯¹"û3FGL J0755.2-2633@ns-8Go*?ë©÷À9.wAýÀ;.ˆcp'?â)¾Fïu@(ä±ÅàJ@ÕÍØã\¿åÕIJ̬ì¿ç¯ ùN#é¿ë°ƒëÔÇ¿å['²ãÉUNASNonenone?ï¦rŁ?žÌvÓZÑ?œë1§OÝ?žÌvÓZÒ?Û['`z‰ù?Ób«(¡¯¡?âR>Ï»?Ób«(¡¯¡?먕nGq?°ùŠbÄGF?Á]ªEÊâ??°ùŠbÄGF?éSáYö͘?±"HÙÐÔÂ?Ê°z˜$É¢?±"HÙÐÔÂ3FGL J0757.5-0536@l6BB…@'õŒÒ
ú/À9Á‡ŸœÀ;•úœé°2?ð»¼x@dV7o-	@LÀM£¿äECÃ'º¿él~_½'¿ìf;}{ù¿ïÿhÅ*/îUNASNonenone?땣>ԗ?ÀëÃÍ%rI?Á©s—­¨?ÀëÃÍ%rI?Á#K¬7Ï?ȖßMt$?ë·-ß²?ȖßMt%?åõ;ÑÐV?·~*`=@?Ôˆ\_Sá?·~*`=B?¬÷O(Ρu?˜ætÂÊ?î0‹
sé?˜ætÂÊ3FGL J0800.6-4806@pk"¦óõÀ"·öµšÀ9¤ØDЩÀ;^
œ;4‰¿æu«'	@fÚÄT®@|ž_Ñ÷¯¿êˆ5Nt	ñ¿æ"Hô‹¿èb"ˆª"¿ïÿ˜ÞL•ÊUNASNonenone	?ïé= åˆò?jâ¾àH.?fÂßw
þ?jâ¾àH)?íÆÜx§'}?»ñœºTÌ~?±É:Ãl?»ñœºTÌ~?íß.pô?¢U|•<?±Œx_o§?¢U|•<?CXÌ ?ƒ×ñAHX?ˆU¯)Ì×¼?ƒ×ñAHX3FGL J0802.3-5610@pÞ䣃'gÀ*YÛ©¢fÀ9ÏCŸ'À;w|ÚQ?ô —•Ž•@VϺ½Ö@í a´Ñ¿æ]†,n6Ù¿â:½h€Çç¿ë–‹¥|§¿îÝЮaZlUNASNonenone?g; 5Ú ?h–ý>>©Ü?ïèÄßÊ%á?h–ý>>©Ü?•¹rD?®²}‰í?ïWB7/<o?®²}‰ì?¾´Òõt?ªÏYÂØ?ì)e¡]с?ªÏYÂØ?¥¿]ŠLÖ?"â#sL÷"?î¤*'[2?"â#sL÷"3FGL J0802.3-0941@l½XdE#ö@%òéhSÀ9ŸúE«Û»À;ŽŸ±m¿ð·¹Ù&w@¤gÕ&b•@A¦`|l¿äÅMíHÃ=¿âøœ×Å+÷¿àРÖÇû¿ß×çõ"ŽUNASNonenone?ïÈÿ˜Ú–?ÊÇÊS?{ö€3'µ+?ÊÇÊS?ï¿ç5ZÈ?‹ÿ<ïOáW?€2©Mü=?‹ÿ<ïOáW?î±ád1Q®?›'ߟ(6?¤áé¼êå?›'ߟ(6?ïãeˆ}´/?lÄETI]Ù?lšw'KÐÍ?lÄETI]Ø3FGL J0810.5-5214@p±´êJŒÀ$L`Ÿ±À9NeÜÓ«
À;E"äE?Ù¹e'è
Ò@\¬ 7@f"_ ¤{¿æÃǞ`¿êÖ!"VˆÅ¿Ý•ôgµ4Ä¿çø¡¨ör§UNASNonenone?ïô(ÇBJ!?e:à²%ƒ?W®q{kÀ?e:à²%"?쑷¹Ÿr¶?¡PÞ<f¡?»rB3jT?¡PÞ<f¢?îrbò¡&'?ŸøUtH?¨ÙÐÕí—á?ŸøUtH?ìÙíz	?¥^£Rs?¹7ð"/·î?¥^£Rs3FGL J0813.5-0356@lG
Ø/×^@0C#À:ZPÀ;µ©FµÆ÷?æ4ô9´h@ÁìóˆÎE?ú¬_©÷¿ïû^Õ¸?ï­Z®CÂ?•ÉæÁ7¿ÖIWé9ÚUNASNonenone?ï÷à nŠ‰?LNñáa0?P>¿"êìU?LNñáa0
?ï£>Û Áo?·@[îM?‡0I7Ϥx?·@[îM?ïm1qu4¯?ˆ*uõÈóa?'YÑÑYj?ˆ*uõÈóe?îwà›p3É?¢ìÇ©Û¸?¨öHüÁ?¢ìÇ©Û¹3FGL J0816.1-5044@p¤´êJŒÀ!9¨Íê>À9«aB:7À;#þT.U~?ôŸY÷î
º@=FŸ¡›q@òÙ æ[¿á‰3hH¿çNM;®=&¿é
ÂØŒ[¿í'íõUFUNASNonenone?"2Wr²?"¦^>d?ïfo½Djo?"¦^>d?±¸ÆÖ‡?½œ!Œ–L1?íÈç%=Ï?½œ!Œ–L1?Õvs‡?µßr¦mµj?å~óDöF<?µßr¦mµj?­lR@ғ?"Uՙ§?î):Ûþ'×?"Uՙ§3FGL J0818.0+3237@g²(¡ß¹9@?WG²JÀ:8CÔk&ÀÀ;çÖNUο©¢ñ^¶öu@!¹f"‡Ý@q]À¥w?ç:¡f—Ž§¿é©a¿Õ$¾í!g?¿èaFNm÷)UNASNonenone?ïÿHw21?»OÔG?ü¹Â³?»OÓç?ï½ãn ž?†Ž~¿KxJ?€‡$yWؖ?†Ž~¿KxI?ïæýƒˆ?ˆðɆ$(Ù?Œ†\€Ÿ?ˆðɆ$(Ø?ïÑöæY?nÜo½<ä'?wŒðÓR?nÜo½<ä3FGL J0823.3-4205c@p<†DR?hÀâøæ0K!À9‹j˜û)À:»Þzt¿ñŽ;AŸˆ@NûÆ_u[@~µÀ@ÍP¿èBS¿âÕ­›rü¿æ¹Lé×cm¿Ðõ›Ã?…QUNASNonenone ?îv¤G¹;^?¬òYäŸÑ¨?¨•»"lJ'?¬òYäŸÑ¨?ï=‰ûò?®äßvp~¯?˜\ŽÀŸ!ç?®äßvp~¯?ìU€€'É?­Y ]p—?¿íSûûq·?­Y ]p–?ïý5f0IË?<9Ùƃ
¤?6TÎ}±¥Î?<9Ùƃ
½3FGL J0823.6-4838@p"HýŸÓoÀ´]+TBÀ8ö$"]?vÀ:ó¸°¶Ñ?õAš	.Ï@þdRåÖ@æW_¸Lb¿à«l	¾o½¿ëÝüÓm®¿è8¢ÆœS¿íOÂNÞNUNASNonenone?ïv£(c›8?"Ÿ–6²­á?'+šóŒ˜ß?"Ÿ–6²­á?è4²(J?Ï#p$š3?Ϗ-7_þÚ?Ï#p$š2?êªcK%mò?°$D`o€?ÅVrÓjH;?°$D`o€?ãpkZäŠ?¶¼m¦Bo¤?Ù)J6ëÅ?¶¼m¦Bo¤3FGL J0826.3-5056@pµìß&k¥À…ñ¾ôœõÀ9C¾b¦¾EÀ;*Aç+ä?ð¥YEÁ€=@a…'ͼ@ÓÖÀk•z¿æo0m
Ó¿È©ü¯#Õ®¿á¡Ôñα¿ïþCj–fUNASNonenone?¶È˜¬Ìò?»Æ‡ZñZ?í/Æìêfa?»Æ‡ZñY?¹•ªƒ~b?Ä-g³0?ìÍJ¯Ÿ3?Ä-g³0?ÉÀÓÄPV?¶OÙÃÑw?éËëüê?¶OÙÃÑw?ÏÓùVmÚÏ?³×‰v(Z?èªd‰M?³×‰v(Z3FGL J0826.3-6400@qfþ=ÁÀ-L4"…ƒÀ9õVI¸±À;­i#L5¿÷'Ìg¢%¯@…×Sƒ¶@¼tÿ[j_¿èš¨
ܹ¿âs? (ÿÔ¿ê#2X(c¿Òpå;¿¯êUNASNonenone?îÝÿ¼d?¦ɋðU…?¢/¤9Å?¦ɋðU…?ïÊ+Á?ƒÙ?†‰Þðˆ?zê`>¦?†‰Þð‰?íèl:)û–? 'åd.ļ?°¼ž.°#R? 'åd.Ľ?ïù)LKÿ!?N¿´S2?KZÎÐ{Ô?N¿´S'3FGL J0829.8-5239@pіœ#·•ÀªB9`tÀ9rƔ¤gSÀ;:?wTW?×Ú+´RœI@
€ˆ!ö@}úÿåþÍ¿åöR­!¿ë½²8Ýþ4¿â5Ài;'¿èiÕ°ïUNASNonenone?ﰋ}u•Ô?‰jx]ÁÀV?ƒÝ ¢š‹?‰jx]ÁÀV?è×S;bÄð?ÎãVò"?Ì¢³tìD?ÎãVò"?í]®Gýa?¦"ñ:ß÷U?µڍÀõ?¦"ñ:ß÷T?ê¶ÓE½ÌÒ?«ÐáCÚW?Å$²é̸?«ÐáCÚW3FGL J0830.5-4452@plÎp:ûÀ
Nb®•ªÀ9ò"Ýr6À:0‰ÁµA–¿ãö¸%^
@‰ÿÈ¢œ?ÿ9{ßto>¿éP¥:üD#?ï½jòŸd?Óa°¦Ûj¿èF¶]I²&UNASNonenone?ê-¦LZ?É?CÌB	"?ÇIg²Î—â?É?CÌB	"?îÿÁ™Žw?±Øùnó†)? æo7?±Øùnó†)?é* 'Š•ô?±yls¯?ËW}µÕ¨3?±yls¯?ïôO'–1õ?ˆ[Üg"hz?W`úӜ®?ˆ[Üg"hx3FGL J0830.8+2629@h­>À//˜@@F¾œˆacÀ:-Ü^:GúÀ;Ê zÉʺ¿ÒŽAX²@&@HNx^@tPÿ÷Çw¿ækš
+í¿é*l{¥¿ÜrWÙcg¿ïÿᘴ(UNASNonenone?ïþ«äqo?5œ§\‹+¢?%G!¸é?5œ§\‹+¸?ï_ën¾²?˜EnhQøT?"ŸÒ() ?˜EnhQøT?ïaË3{B?Žïô¤y
?"Æ™—½Z?Žïô¤y?ï@^ú@¬?…'«Ü0±?Œ¯èAoÕ"?…'«Ü0±	3FGL J0832.8-4321@p]1¤½º
ÀzMÙ§¦£À8ßÕùµcÀ:p•âTô?çžR@i§Ž@¾½Òß@`•ì翌»Ë'%Þ¿êFÑËå¿éô{Kû¬¿ØBR'X"¦UNASNonenone?֙Måc¡É?ÌçàH{B–?ä³Y
N/?ÌçàH{B–?éÜä¯Ñ‹?ȉ.aXK?ȏðm@¹Ô?ȉ.aXK?à>|kœÔ®?½Ö3TáAž?߃(ÆV¤?½Ö3TáAž?èÏ1!V?½t&Ϋ—°?ÌÃ;{ù¤?½t&Ϋ—°3FGL J0834.5-4825@p¡JB®Ñ9ÀV¿2/'À9hhó ¸À:Äþí±Hã¿Âï÷<j
@Áe¥÷ @€w´—¿çŸÊR@Œ¿ê¤€HBl•¿ÞŠz܃èÇ¿êl¹oUUNASNonenone?ïv:F×ý?¥¹õA¡N#?Ÿ'8·%h?¥¹õA¡N$?îê¼8fh?°
eu«?¡^$<y™t?°
eu«?ë{¹å@Áè?­"˜«£?Âjüø`?­"˜«£?ܖ&Ë?‡?7KfN?‰ÈÚvM+?‡?7KfP3FGL J0834.6+6101@cpŠGìþ›@AõÑN;Í6À:'dgˆ¥VÀ<
n.±Ä3?Ғf)T¸@Ëg!wI
@S;ÝÛ¾¿ÝpÑF⛿äpÓàx"¿ê'ÃC-ž–¿ãM®23ËUNASNonenone?î´Yëb÷?°½êóÅø@?¤ºn±IД?°½êóÅø@?ì^j•6Šw?Ä
¼%c±?½«VK¬P?Ä
¼%c±?ëŠö:ygè?²¸ëµ7?ÁÔ'``?²¸ëµ7?æ sLö²‡?ÀZêsÒ¯Ú?Ó¿fšò?ÀZêsÒ¯Ú3FGL J0838.8-2829@oS\gßã*@4~êÁªÀ9©Û0=À;r-͘¤§?òMÂÎq<®@â†óNÂ@ÌÞࠔ5¿àth‡©¿àƒ÷à"¿äŒÌV°;¿îG\sQUNASNonenone?kBºò?dÀáOQ ?ïäo½E
ò?dÀáOQ ?«¢¿í*¥T?Á{tELý?îEÔ-Uª?Á{tELý?¯'Ô¶L¶?£ÐOÙ²õ?îÒ¾4›4?£ÐOÙ²÷?¹ ^oVm?›p·`Ë"^?ìÛþô23?›p·`Ë"]3FGL J0838.9-4056c@pI*â—9m?Ó@¦¹<ÍÀ8Ð/9©núÀ:mSB3'?Ä\G‹|Aç@Ù@ºZYh@MüŸù/+¿ç×{ÉÇV¿é' ÚE¿ë³3§*¿æâÓUÁÂFUNASNonenone(?êb6Œ?n{?ÄiU?Æw%ÏF?ÄiU?âNŠãň?ÕÖ{SŠ6?Ûbê8uèð?ÕÖ{SŠ6?æ?âç¥xn?·
ÂG|?Ӏ:0µ%?·
ÂG|?칕ȹÛ?°€ä‰‰õ+?º3Q¿Ú1!?°€ä‰‰õ*3FGL J0843.4+6713@by•$Ý@A͂¡ ÏÀ9¦sŠ;WÅÀ;Βßk5?çÌ'æs@uÞ©n#?ÿàß=Ù¿æÑ´¬ß5¿Ü¬È$òRÿҜz¿;Ù¿ìº9$
üBUNASNonenone?çCnXœÇ'?É [è¼2?Ñy#NÆpü?É [è¼2?ä›Qs¯Ó?ÑoR¥É?ÖÉ]àZ?ÑoR¥É?åüZé›ß-?ºÝEy—¸?ÔJ,ÈA¦?ºÝEy—¸?ç§<•´?¾¼lúÇQò?Ṉ̃õ†Ô—?¾¼lúÇQò3FGL J0844.3-4741@p§Î_oÒÀ¯ŠúšeqÀ9
£oÜ0îÀ:œÖÒ	L°?ì%p|ê·@H©}è88@±>ÿo6o?ïÿ¡"uÿr¿æ%ºÃϑè¿çŸd}G¿ìZíß
Ž€UNASNonenone?âK"c!ۍ?׆y']·?Ûh÷9¼Hå?׆y']·?áþ¿·Å?Õs3nÆè?܁û֐w?Õs3nÆè?Óg'•	£Ù?¹´]Dæ"ò?æL6µ{.?¹´]Dæ"ò?Ü2Fç¢Û?Àæ
qB¸?áæ܌x®'?Àæ
qB¸3FGL J0846.8-2638@oFÅCk›@$ªkøvžÃÀ:–ç7²À;œ}>ïÿØ?˜ÌÖõÕ@Ð3f´¿æ@ÈX *,y¿Ý´…XDοëX
Ò?l@¿ïÿ™]-š?ïü…û4Ç»UNASNonenone?ïíSN±˜?p†dß"þ@?b¬±NgpÙ?p†dß"þ??mÈþv? 6PÑˎ?€œûÀby? 6PÑˍ?íqüMNs?§Ê‡g¬Í²?´p—åŒg?§Ê‡g¬Í²?ïìBÑü!j?qót~b?c½.ޕJ?qót~b3FGL J0847.2-6936@qÆð:û~'À0@ ÇÀ:Å~#òNÀ;¹ë˕•(¿õ¾"_¦XÅ@™ýAµ@4÷ 2z|¿êu)6Òqt¿äëE
¡¿¿ë	õûÖ`Û?±zG(ÒiìUNASNonenone	?ïù_w	t,?MçE`(Õ}?J'#Ú/Nq?MçE`(Õw?ï×ܛ½Ý?´¼|ò"?t²!q'¢?´¼|ò"?ïaòrý;?Š€T·ßn?"Á± X'?Š€T·ßm?ïÿvéõõ?¯"?þÞ?"Á^sò?¯"?þ©3FGL J0848.2-4524@p'3]$žE¿ò.Ñõ*¹èÀ8Z¥öŸ..À:AJFu/W?Ü[wµn6i@*°ÁÔKF@:3q¿ãΞÜØ¿è‡Î¥%O¿çÚ¸'›¿æðu̓tšUNASNonenone?ҾݔÀ;?Э^óÍí?树5Ÿâ€?Э^óÍí?àgèú<3?ӂá¾5Σ?ß0.†ý˜?ӂá¾5Σ?ß¿_i£e?À›®Ò~:?à PK.rÍ?À›®Ò~:?ëqF2d?´¥døX÷ô?Â;êç7–m?´¥døX÷ô3FGL J0848.5+7018@brGE8ï@A•"Ý—ö+À:€€VÒt¬À<i[
lÐÀ‰©6šœ@ýïÀí›y@eÀy,g?ÏM¤È½|¿å[¦‡ÙL¿Ö0«±LO¿ãl¥‹«UNASNonenone?ïÿPm¯Â?"4v²!?òJ° ž?"4v² ¾?ïØZí	?€J…øü7?s҉1|{¼?€J…øü7?ï´ÿUYå?'ioeË0´?'À*º)†š?'ioeË0·?ïÿ÷Nâ>ßX¥ÝrZ>ÑÝb;Ìw>ßX¥Ýo@3FGL J0854.4-4404@pŒîËûµ?âRuÚÀ8"­¨DWHÀ:DUFƒr?êOI£Ú\¥@¤'šG@Íù ?{¿âªÙ-5ö»¿ê"¶Êh*¿ëÅýÅ_'"¿×1¼áUNASNonenone?Ó&ƒ4¯! ?ѶGà<?æl¾e¨o/?ѶGà<?âŒÈÝN#–?Ô&¦Jü•
?ÚænEc¸Õ?Ô&¦Jü•
?ÚpéQw‰?Â{Y@8§?âýG‹WD;?Â{Y@8§?ê}*$™î2?ºêÿÈ}^¼?ÆWm˜G9?ºêÿÈ}^¼3FGL J0855.4+7142@aÄû~ÿ—@Aœà\̉±À9²õÚPÀ;¾½Žkh.?Ê*êdbU5@_ÝË¢«;@"5`4>¿âÙ±8¿æËÜ2¬‹Ë¿æÆCG¿ïÿêaïD'UNASNonenone?ïþ(õ߅'?1"PÅFÈ?-p¢­…í?1"PÅF½?ED´?¤BÕ7 0Y?¤‡;«´µ?¤BÕ7 0Y?ï¿<µ¸R-?|qÖç'$$?€0ґët»?|qÖç'$,?îááh†?Ÿét~Šª™?®áé~'œ?Ÿét~Šª™3FGL J0856.4+6429@bÔ_Eà´á@BÏ …±…IÀ:wÖ²ÿœ-À;þ¿:=°¿£	ëû·@±¯ØuLˆ@iƒÿÔa¿ê_]Zùö§¿áÎÂ7óaa¿ã=ÞNn;â¿âˀR[þ•UNASNonenone?ïúEˆÛ¼?R"³sæ?E¾éܑy?R"³sá?ºL_b?–´d§?XQlè'?–´d§?ïb .]³?Þ•µÆ¬¸?"«ú4IŸ½?Þ•µÆ¬·?ï×¡á,Á?€ÑCu""µ?‹Ê‡´Ï¤?€ÑCu""¶3FGL J0858.0-4834@pÊÅXd¿þc@A8¯À8÷0t<ÿÀ:T¹¼NÐH?ðjÓ*‰ìR@
âjé,)@•ô@")›¿é¬p®i¿Þå;j܏/¿ízíBIb¿æ#}"ÔÕIUNASNonenone?¦è'~®UH?¸ú;{¦8?î'wØ«?¸ú;{¦8?ҍDWõ5?Ï<ޓ(òQ?æ¹]üTe?Ï<ޓ(òQ?Óµ±†êPw?¼ƒ<+‰‰'?æ%'<Š×Å?¼ƒ<+‰‰'?ЁHîðÃË?½dnÓy¹$?ç¿[ˆ‡ž?½dnÓy¹$3FGL J0859.3-4732@pÀ
»Då¿ð¸±§­X"À8±öFBÚpÀ:J­wœï?ëñ&D§Ã@
2L["e†@^¡`^x?š¢öÛ+C׿ërò·~B6¿ârKuãö¤¿êM|œÖUNASNonenone?¸ùFQTR?Á¶XRÀ?ìà×5Õu¼?Á¶XRÀ?À¾"äaue?ÅUñbìÆù?ëÐ[碦?ÅUñbìÆù?ÔB͎'?¸ê07×­W?åޙ8þ6ø?¸ê07×­V?Ö$jžS?Àèãdw;?äíþJ°Öq?Àèãdw;3FGL J0900.0+6754@bL"‰a=@Buk¹Œ~(À:ùÂÏ	À<´æüù»?Чɧ‡@©(ÃBµ\@è¶à|W¿Û|õĒÁŽ¿ä7æN†©[¿ÜÉnûØ b¿ïÿ™äOUNASNonenone?íbm Ë'‰?¼³a£)]§?´ì'ù£k°?¼³a£)]§?ìÞ
3{?º
ª¾'þ÷?¿—æd)?º
ª¾'þø?ê™ÊºC!?¶«XÇæ§?ŘÖó?¶«XÇæ§?ìX¤ËE¶?®Wnf)ô?½:٥ӂH?®Wnf)õ3FGL J0901.0-6725@q·}'ÔÀ+ˆ}€^_1À:D!BoçÀ;ºÉ«¿ñ0Ìxéö©@
AK<>u@0ـ9vC¿æS÷'.|{¿åƒéY€ú¿è-h+•¿äGïç?PUNASNonenone?ïîñFb……?e'Á3ã;M?a¹zzC?e'Á3ã;N?ïÀq^<[h?‹r¥¶'«?ÇPáÒKö?‹r¥¶'ª?îúÊ``ºu?'ÆR
±h? SYùôX°?'ÆR
±h?ïðÂVÈ~ÿ?Zx~Æ?^{RoJ?Zx~Æ3FGL J0903.0-4826@pÑXDЩ¿òÛç‡c60À8ÓÝËø'wÀ:Y8Ëùh6?õ(Ve½I!@
3´k×êb@¼2@·?ê?sÃq.k¿êIˆÆÒP´¿èLd¤LD¿ïÿæ
æÀUNASNonenone?Âen‰_\?ÇðÀÍ]u?ëz&¤]¨)?ÇðÀÍ]u?€	ÁЏza?•¤Ð·fm?ï¿Øø½Â?•¤Ð·fm?ÌH²hm,?´À<qbë•?èíÓ{åä´?´À<qbë–?¯Õ"hÃ?¡ÌʊJ‹?î®è¹t?¡ÌʊJ‹3FGL J0903.2-4744@pÉAÝ!ê¿åߑ€EŠ¤À8­XIm1\À:\ƒ‹:[F?óšzí±ô¯@Å·n–¶@Aäpb¿ìˆÎñÅ+?Ð$fJÑyI¿éKÉ®¤Ÿ¿ç;ý8>N´UNASNonenone?Ð6mçgT?È /BMÕ
?çäÉ}LV?È /BMÕ
?ÏÏÎe¥ó]?Ïæ2Jë:?èf–ƒ(?Ïæ2Jë:?Ýç4‹æVð?¸c­À€$?áeºԇ?¸c­À€$?ۘ)Uِž?Á9´h'ß?â3ëU7°?Á9´h'ß3FGL J0905.8-2127@o'>E@0òædM‡rÀ9›†g­ÓÀ;}´{/P?ó6Qbô@xè±Ú®@G—¸òпàÍ,×Wû¿ê~²Ó¿éù{ßýߝ¿ïÿJX=ÙªUNASNonenone?â1{§É^?Ìû²I•?۝±èmC?Ìû²I•?ÒF'Ø}?жü8[L.?æÜñ7r"Ã?жü8[L.?áÇ˧ÌD?·ÄªÂ\ô?Üph°gÛz?·ÄªÂ\ô?±Âj×*ê?›ÅtÓ Û?íDz¼%¢?›ÅtÓ Û3FGL J0918.2-4859@pó¿3‡?҉O_
ׄÀ9.‡¶BFÌÀ:¥£Ho?å¿ÖQ¶@
ÀÍ^m»@†Î¿Á œ¿Ù Ö²÷¿æÒáìĎæ¿ç¶hK2¿èýI¯vz±UNASNonenone?ÐO¼+_'?Ì÷˹]üŽ?çØ!êxP7?Ì÷˹]üŽ?Ñú­é®?Ðn~X&i?ç©(ñ²?Ðn~X&i?ÛÄn÷n"'?Áÿ ÅY¤?âȄHµ¿?Áÿ ÅY¤?ãsa#Œ‹?¾b}døô?Ù=¸çÂê?¾b}døô3FGL J0919.4+6604@bvwFˆ{@C¬ü'œýÒÀ:§¢m}±ÝÀ<»%}¿ËDzfoÈ@Øi2ɀè@DÀ
¡©¿ÞºÎ}Q¿×:´Z¿Þï`qH±¿ê÷Ø'D,UNASNonenone?íb>%F^?¿˜/Çfj?´î×=Í?¿˜/Çfj?îì_ËùÁž?¤®0Ë3¨"?¡:@cæ#?¤®0Ë3¨"?ê©ô‰ï
L?´A3U‹cí?ÅX-ØCÖÐ?´A3U‹cî?ïL'¾Ž?}XAëO?–|ü›.1?}XAëN3FGL J0919.5-2200@ol¯öÓ0"@3áÞ¬É!À:qÀY÷ÃÀ;¾UË
¯ì¿Ô9Þpì¯Ê@ÿä8¼µ@"ÔÒXR¿ïûM˜†–?ïMÁ`KÞ꿬ŒáõÆ6¿ïÿÚeÌUNASNonenone?칒œõžs?Æ!6Ãs?º3kSm?Æ!6Ãs?ë7L52"?Ð
	^²?Ã#âÏ+5°?Ð
	^²?æXöۖ½ç?æŒ×¾}×?ÓNH҄1?æŒ×¾}×?ïfnð¢Z?ž@>þ4£_?"2!ë´¾ð?ž@>þ4£`3FGL J0921.6+2339@iœ´¢3œ@Ej˜þi'À9ØüvÀ;°jš¸¿ãðrô
Ë­@FŠ{ïd§?ÿ¢Z± I¿ÐÔò׿´¿áéÈ]ÒC.¿Ø¨b†¿ä<+{.œUNASNonenone?ïøßp¬8Ù?VÎÞw¶s?L'=Ožj?VÎÞw¶v?ï§Æ6Ë?"V}¸Û?†?ÎzrMT?"V}¸Û?ïv°ëeü1?‹®ŽO¢KS?')â"@yé?‹®ŽO¢KP?ïñ{¶ãú?YºØÚ®9?\á'8Î?YºØÚ®93FGL J0923.8-5154@q=ÈK¿òS;C£À8Íg<O;§À:ÊPrß?â ¸tu7@
GWŎ¿÷@`t	¿ã³íÅ벿ëuÖ?!¿äºáÊ#¾æ¿èÌPi`'UNASNonenone	?ÜáùÜÇ¡?ШcôŸÝ?Ꮬw/?ШcôŸÝ?ÂÔ샙6?ǽœÄz¾?ëJÄø_²?ǽœÄz¾?äs¤Ž6ô?¼Í"/<Ã?׶ã'Ñ?¼Í"/<Ã?܈!èGOÁ?»ÚuÊc?á»ïÜX?»ÚuÊc3FGL J0928.3-5255@q1MjO¿ötڂ—õUÀ:_UÐìíÀ;<ÔL?ßcOüÒ@¼HKôL?úgΠ·p¿Ð¶*
ðƒ‹¿ïÿ÷Dx2Ÿ?ïþñå,Œr¿½s54rÖëUNASNonenone?ï÷Ö©w?Y¶
['ð?QîR­̑?Y¶
['ð?ëî%nfRT?Ë–¬‰Z–?ÀGjFf¶¯?Ë–¬‰Z–?ï`ê7x¨?Ë	Qg€?"â¹êÿp?Ë	Qgƒ?ïý"ÄqHd?T.²¡à›e?3aÜu¼Ü¾?T.²¡à›b3FGL J0930.7+5133@d·—xW)³@F®$‰LD|À:ÊA{ËRyÀ<!¡t­¿ç'"'åw>@îÔ&2n½@‹ù€_
ý¿è‡>—Y<K¿Ô/¼«Âf¿ÝJ@(l¹D¿äÑäª0UNASNonenone?ïpUŒ"?¡3Áëæ'?'ÿ]µN{¸?¡3Áëæ'?îØX§øþ?­ìi&¦]A?¢zu€~Ð?­ìi&¦]A?î£.‹ñ?¦'Ñk»5?¥ÍN€î?¦'Ñk»5?ï² ÚùpZ?Ú ¾èï?ƒwÉA£é¾?Ú ¾èï3FGL J0931.8+6739@b%M:'£@CâöÕ®À:ZxyŽaWÀ<:§›ºÜ?´>xt鈆@F[oèEN@T1ÿ¬s?¹hBý‰5Ò¿æ	8Ö`Il¿Þ¥LàÙI2¿á7vjP¼íUNASNonenone?ïñKp?í?f§†l€?]i€%åf?f§†l€?ï"6sWŸ:?"™o!T^µ?Žòc*1`?"™o!T^µ?ïBEs@âð?"¹§ÁýÖ;?—·Q—ã¢%?"¹§ÁýÖ=?ïl͘°»?"Ãt03f?'FLéè?"Ãt03f3FGL J0935.1-1736@oOö©?)@8²~
ÇÚÀ:#×>?Ö°À;MPëªÞ?ؾ`Èíš"@bŽëjÈ?ûúp™?ïô¡›¬Õr¿åU›d䠿΅.jC<¿Ý
Wna\UNASNonenone?ïý9Á݂Š?<¥qM{u?61ñ묶?<¥qM{m?寧ûý	?§ï?†~UA½Ö?§ï?ïžû↑U?',y*x?ˆAjÒ?',y*w?îÀþãÒ±´?–pQŽì|?£ðÂÔä¶?–pQŽì|
3FGL J0935.2+0903@lšmÚÏ@D.÷<ÉÀ9àyçLªÓÀ;ÈÓÄ7ÒÕ?õRl>A¯"@׎5bbv@8	cr–¿À.(Q­Ç¤¿å®Wa™U°¿ë™ISþQ¿ïÿÆç'
'UNASNonenone?ë-â'p'?ýÑ9àõ?ÃHu¶=·ð?ýÑ9àõ?Ù´ãÖkÉ?Íà‰YN½v?ã%Ž~"Ê?Íà‰YN½v?ṕ»Ë?¶ƒwâz?܌ԉÊió?¶ƒwâz?ȕ£º[Þ?²:)œåvr?éڛ×i?²:)œåvr3FGL J0936.3-2114@o³ÿX:S¹@6n¾‰¬½À:`'b"sÀ;¹ö¥ä*·¿ð5§=h@ǽµ'®F?ý|@€M?Àømºm¥¿à
¶¡è´¿×¿Y±¿Ü¾¬3á?UNASNonenone?ïô»»ÎÓ=?Zp° ?VˆˆbY…D?Zp°œ?ïÜ/¦Ù?|K­çA"V?qèvs,"b?|K­çA"U?ïwOËg?+?‰Ô1ÖÝZ?'"–?‰Ô1ÖÝZ?ïýid÷YÉ?5Œ.}z¬Ð?4´ØE1µ#?5Œ.}z¬ß3FGL J0937.1-4544c@pô ě¥ã@^']Šõ'À9±aB:73À;A€t.¦¿Í.'¹5@dÆ(Bê@닠\¬S¿í°½wš@¿àMà
õ¯ù¿ßÛ[ž"Þ§¿ÞÛÎJv=UNASNonenone(?ïú;
çð?O¿¹"ˆe?GÈc€Ds?O¿¹"ˆh?ïÂÇ(n½R?Ë+žýéÒ?~œkÈ¡WB?Ë+žýéÓ?ï4êތٚ?"ÚÊb/8º?™b¤.dÌö?"ÚÊb/8¹?ïæ³4'¿Á?]õCr¢?iLËn@@
?]õCr3FGL J0937.8-6407@qºwÄ\»ÃÀ!"Ê`"À9Ó9¾hÀ;…jŸ±
Ï?Ȑ}l£}"@m¼}cÃ@\Bjy¿âRD###¿ëI"×ã¬7¿ã]W</ŽÂ¿Ú^žRÞ@µUNASNonenone?ïú%+ÙĽ?Oȏor†?GkP˜í;?Oȏor…?îŒD±‹y?³ã<ð¨Áj?§;´ïÇHp?³ã<ð¨Áj?ðA™Õ?†Vx$T!:?ŒžÃ?†Vx$T!<?ïfR=Þڅ?ƒÔ{.Jj\?"5¸D$¯q?ƒÔ{.Jj]3FGL J0937.9-1435@o8ÅCk@;48L`À:Kç]qËÀ;¹¤½º
R?ãC^ÿƒ@j3PåJÈ?þ<¶úS?ïý:"£§¿Ù"´¥Â%¿ÚÁlÇS'"¿è°Iۅ9UNASNonenone?ï¥qc4iÇ?'âxÚZ‰?†£§2åŽ}?'âxÚZ‰?îÀÑõÝ¡?¦ £Èªw7?£ÿÒà¢%ñ?¦ £Èªw7?íƄòIƒö?¤—È–ùP?±ËØm³àJ?¤—È–ùO?ìqb™J›?¬ï?….Ô?¼të5«'¨?¬ï?….Ô3FGL J0940.6-7609@rCóÿ¬*À1lÙÆ°SÀ9?ÎÞ¨À;tOÞd¤Å?½)7ÿD7@ÚÂ-âf@H_•;ç¿æðýlŽõ¿ÞG¿myç¿é›ã±¿ïÿۄ—÷%UNASNonenone?èüEߨ¯?͕%Ú´N?Ìè]Cí?͕%Ú´O?Û×k¯$,1?Ó14kªqì?âJ(méè?Ó14kªqì?á‹-ÇHÕÒ?¿u?'P\í?Üé¤qnT\?¿u?'P\í?äÅ $go?ÀbšêNYv?Öt¿·õ1#?ÀbšêNYv3FGL J0941.0+6151@bïu£KÜ@EŸÝ]=ȸÀ:€º¥'ÜÀ<
±qýs^?Ú9üSUÆ@¾{
L¯@_"ŸèN¿êô
$ù)¿âe U,y¨¿Ö¹âÏÃw9¿è–ËFm€?UNASNonenone?ïÚ6á‹\?}7U7¨?rätºQ™?}7U7©?îÏG»™˜?¥§C»£ŒÚ?£"Fg&–?¥§C»£ŒÚ?îÚ®Ô£?›L¶Yéj?¢_ŵÇ?›L¶Yéj?îJ!ŸÙÜn?›wã+»ÝÀ?«]æb9-?›wã+»ÝÀ3FGL J0946.2+5209@d7Ÿ©~@GÁÊB®Ñ9À:/þ|rAfÀ<ãðÖ?ä²]Lƒ³¡@ЩIëñ@á'uƬ¿ç/ϓ ¿ç:`ϒi¿ïðŽºå»þ¿ïó¨d@OUNASNonenone?ïæ³A"®?wny/:òœ?iLô¾{R??wny/:ò?åÑٍ'}?Ï¿ »Ç@4?Ô\LåÛ±?Ï¿ »Ç@4?îÄo8;?™àr'ÒaQ?§ã¹|OŒ?™àr'ÒaO?Û‹Qøú~?ÂeuÀbED?â}:W'Á?ÂeuÀbED3FGL J0948.1-3641@p¬/ƒ{J#@)üõ:uGÀ9N]-؀À;"^‡tÔ?얦/ݛÛ@gĹWúé@Æï¿kn¿ç¥ASÈ¿ê÷˜lÀ?¿åJªn÷¿ïÿ²,(UNASNonenone?狼?…?¢c|CŸ"?œ\Kj˜y?¢c|CŸ"?Þæxã}ª?Ñ@ÿVÝs¨?àóŒÃŽA+?Ñ@ÿVÝs¨?ê
2|Ì»†?°Öh'X|I?ÇË6Íå?°Öh'X|I?ÏðÛ))?³Fæè/«?èù;‰5¶?³Fæè/«3FGL J0948.8-4243@píƒ<`Ÿ@ û¼ÓZ…ˆÀ9ª¨ëF4˜À;u­Ñ_Å¿Úç'euz«@
;R'rY@ñ…@œ'h¿êeÜVòD¿ã9¾dv™‡¿ß0…_a¼¿ê(,"dËUNASNonenone?ïsíËuÙ?•¬¹ÊbI?'BF'Då?•¬¹ÊbI?ïHÿ)«ºh?¤ÚE†ywà?–àʈ³	?¤ÚE†ywà?ìNJÿyî!?§"d^0—×?¹Ã¨0Žû?§"d^0—×?ïph¢=£˜?‡Í¬v$Ze?'òë¸KŒþ?‡Í¬v$Ze3FGL J0950.4+7550@`í(Œç°@BD–Ý&·$À:Ö`"•À<=%ÑJàÏ¿ì1Éc‹À"@
óp˜nv@'Í@¿èòW‡´¿ã¡ãÙ?8¿Û™;‡·ç/¿ã¬¬
VèfUNASNonenone?ïá®ì¿µ?‡Ê&jl•+?nQú@JF?‡Ê&jl•(?ï¹Ý"SÝÁ?ˆ}/ÂÇl?ˆžëÆ?ˆ}/ÂÇl?íûécA{²?ªµvKTF?° ´åô"j?ªµvKTF?ïò%4Çþ1?ZôóŒáƒè?[µ–pœÆ?ZôóŒáƒí3FGL J0952.8+0711@l·`—Ì@E¢}sÉÀ:sÐIYÀ;µ™9øI?Ô£xM¢'æ@
jT»ï?û0©ôg?ïùcñÁùµ¿ ['îËi¿×®k@sk¿Û~ˆ&ÌëUNASNonenone?ïè¤|&Á?q#€OÍå?gþ[ƒÙ?P?q#€OÍä?ïIù&¹?¢'$tyhƒ?–߀Þ{(Ô?¢'$tyhƒ?ï''*Á?"ËãÃí͸?œ;
Ú§ß5?"ËãÃíͶ?î¹íC"Ê?›î"Ž@«"?¤a+ÍÓ^?›î"Ž@«ƒ3FGL J1002.0-2837@pyæ{_ï@5¸Ç\J"À:*ˆ«€À;µØÿàöO?çÇ(¾Žñ@GP×3@œ	ßý¬?ÇVùÌ_>ª¿è`ë'UÚR¿é!ÉÔIï¿ïÿB¸·AUNASNonenone?ï`\í$¯x?ž"F¾Èˆ?"ôb[jø?ž"F¾È‡?Ùرvܗø?ÐI/³šB?ã§D'´?ÐI/³šB?ë	!øÒ¢?¬»oL@?ÃÛzµy?¬»oL@?ÎÄ<GUT?³‡ÇApÛ?èxÎðî*¬?³‡ÇApÛ3FGL J1003.7-5215@qlKƧïž@–ÎãþAºÀ9Æ)É'%ßÀ;7]ig¢§?íb¹æ±6@˦‡Ù@{>ŸÍæ'¿"±h~Èô¿Üþ?FοåµjlÒ³Ž¿ì•h.èuËUNASNonenone?­ïV/!ˆé?°º]3?p?î!

çs?°º]3?p?âÌ_RZŸ?т˜sԒ¼?ÚgA[÷JÄ?т˜sԒ¼?ڗ鮙Ä+?¹"°¬­>?â´(³ê?¹"°¬­=?ã#¨ékº?µÙXt¹?Ù¸®-)‹?µÙXt¹3FGL J1008.6-5706@q£*\|Ù¿î3†_€>À8&Ô©À:(ÇÅüÎó?ÛbÕh¸âE@
Ÿµâûba@ˆ€—•¿äúEoº'Ñ¿æy™¨s¥¿ëAÀáÿ¿áŒs%¡UNASNonenone?Á,Bip2²?É¥(ÿб?ë´ïe£óT?É¥(ÿб?ÔM®ÚM^Ë?Ò")ñýP?åÙ('ÙP›?Ò")ñýP?ÙÖ/™-i?¿ê³ƒçˆð?ãè?3iK?¿ê³ƒçˆï?äßæŸS+ñ?Ä[w'ITÚ?Ö@2ÁY¨?Ä[w'ITÚ3FGL J1010.8-7645c@r`ï~=ÁÀ0¼øµˆãiÀ:¾7ޓŸÀ;o	µ‹g¨À7º¬cˬ@õ&Ûa:@sð?m©&¿ç–î÷ø}¿ê¬kÉ°@X¿åÖÆ]xÐ?¨ž€Íߋ/UNASNonenone ?ïóÄÉ89?_ÍèHèQ?Xvmþ±?_ÍèHèT?ïÚ-ßò?'Ë:÷&?rôöéV?'Ë:÷&?îïQÕ§EÅ?"@s[è?¡
⥋£¾?"@s[æ?ïÿõԈw\>áDfE²w>ÔVïFí>áDfE²c3FGL J1013.4-4008@qRÇ%Ä@*µÿÅGÀ:=©µpµÀ;ª\™'6¿àvÃá@3%>Röó@Æ ‹:Ü¿ãM-M:¿èw/òêv_¿Úzƒ9L¿Üщêc®UNASNonenone?ïýûh@¥?2SÀCÁ	‰?0$½úӀ~?2SÀCÁ	Ž?ïÙFÉË[Å?}É-<·™1?s\›R%?}É-<·™.?~ÁÐT?ˆwe "?‰`O‹êÝ?ˆwe !?ïí¹O¨#L?]HL'Ƴ²?bF°WÜ´.?]HL'Ƴµ3FGL J1016.6-4244@q/È÷Q@'%WšñˆnÀ:#ÜHjÒÝÀ;'Uœê†ò?á;Ó*½@x|¦CÌ?üƒÒÀVǸ?ï±jØÞJp¿ãæh4æe¿Æáâ	í6¿Ú0âÿ$tUNASNonenone?ïþ%†6h<?0»×;d§?-§œ™|:<?0»×;d¥?ïÆ.iz¼?‡!Ãl™T
?|èËBö¡ˆ?‡!Ãl™T
?ï­ÉÑ+Àf?ÁÔHxéë?"‹µæP?ÁÔHxéî?ﷅDÈd?uóÀÀøp²?'¸.Íç?uóÀÀøp³3FGL J1016.9-2653@p"æ1ø @8sÀµgUÀ:ùã†MÀ;ÁSL®.|?äøã#%t@F,6ê¢Ì@×(Ÿ[zz¿äšèù=f¿æ
Hy&Ä¿ê²!óR¿ïÿå|WO®UNASNonenone?ïߺ…µÐŒ?r{X•I/Ô?p"½%¹¸?r{X•I/Ö?ækö*3D?ÉÊÂô y?Ó(«™ßx?ÉÊÂô y?íãâ'ž[‰? %¤Ü.°?°àîÃ
#´? %¤Ü.°?ÙqØ«ڛ?·@k¤]?ãGª}'²?·@k¤]3FGL J1018.2-6254@qç"ßÎ1QÀ'C¦GýÆÀ9–©$Q!À;A#·;k?='9@)ÿæ)À@Š½¿¾œ]¿çXQ¹—L¿ì¯ \†ä¿Üi"Ei8¿èø²JYYQUNASNonenone?íE5L'‹?¹d^múb÷?µÖWM›k©?¹d^múb÷?ÝâõÚG?Õ´€¯ÈÑþ?á|…Üt?Õ´€¯ÈÑþ?ê?RXŽ½?°HµQñÝ?ǶÅ?°HµQñÝ?Ô®bésÇ?½øÉÉõ¡C?å¨Î‹Fs?½øÉÉõ¡C3FGL J1021.9-5815c@qÄó#x«
¿ìùcÞ÷œ¯À8‡7ø"Ñ´À9øîº]^€?ò¬g|õ@
pò\ÔA`@iŸè=A¿ê¨ßp¤"¿èPÒüøʾ¿æ?˜°ªF)¿åX£7ÜUNASNonenone1?þ•Ä-ä? Œ™è+š<?ïHo? Œ™è+š<?Æý-¦m³?ÈoµìŸ«?ê@´–d"??ÈoµìŸ«?̨Ò?¶
27Y6?èùÕúËyº?¶
27Y6?Ñ.Ö9Ï-Ê?À1îly!r?çh"ãi?À1îly!r3FGL J1024.3-5757@qƌ½D¦¿Þ)VÍÀ9š‹1!
À:.Ü:(ú¿Ñ>ø­jÈ@ò¿[Ëñ?þSé Àiè¿î;[¶4/¿åW#P?Å7ÿÒø0¿â¾ôUNASNonenone?ê­L!ƒJ?Æðbë6¾?ÅKâÏyòÙ?Æðbë6¾?èÃȾd;D?Ó°7B´1?ÌðÝoð?Ó°7B´1?èhsJs"N?²®6.BÌ:?Î^2Ö3vÊ?²®6.BÌ:?ï½T™;$V?—B²}{Ó?€ªÙ±6êž?—B²}{Ó3FGL J1024.4-4545@q]¼ÓZ…ˆ@#®šõº+àÀ:dú:þÀ;­â1¸ß°¿Ù	­Ä°ú@
CËPuä?ÿmVàa!¿änkͥݿèëÀJˆdh¿×ÄöCÏÊ¿s)â4d¢UNASNonenone?ïÿw†œ)?`½÷É6,?,Æ·?`½÷É6?ïÏëâÎÍ?‡¤!•ãåÔ?x
x˜™¹?‡¤!•ãåÔ?ïÚîd'?qÑŸþ7?rˆÍ¶÷òœ?qÑŸþ4?ïúO÷›Ý?CN5ì¸V?FÀ!"ÜŠü?CN5ì¸T3FGL J1025.1-6507@r#9ÀëîÀðÞ	52èÀ9g½ò>v]À;OÅ?é$?ð1©J¼'Á@¿r/r^l@Y© ¢ÍJ¿ä48/¶é¿ç
Šån%Å¿ïõ2\¸"?ï!¦mèfUNASNonenone?îÃÀÁš¸?¸\áûk?¯ãÃóæT~?¸\áûk?îœý³r?¸¯WŸrD?¦0.´ÈßÌ?¸¯WŸrC?ê'™	?±$o}á8?Ç·c©›Ûå?±$o}á8?ïTT\Øü?£lP׉7?•|Õtdàs?£lP׉73FGL J1025.7-5659c@qÁ;÷'?ÜÓ¢©ã"À9·
èaÀ:O|N/7ü?è
j®–ù#@U¶öv¿O@'Ÿûž¿ã]+Í}¿ë@%§ô¿êöü²e¿äZW'=°UNASNonenone0?ÏráɄÑ?Ð{	·@8?è#GžËº?Ð{	·@8?Ú#\ëï?Ó*¹J2F?âî1QŠt?Ó*¹J2G?×؄ÞRZ+?Àú†"Ãhb?佐ÖÒé?Àú†"Ãha?ät÷øÚÏ?ÍgvH÷º?×àJb?ÍgvH÷º3FGL J1025.9-5930@q֍"M;¿úûh÷:^¡À9õ@‰]À:vc ¹HŒ¿ù\·%Eµ@`?
1@¼¿Àéz¿Û3_Œò0"¿åT]/¹‰­¿í\ºPüпÏeo+ÃUNASNonenone?ã@ò~ë"?͏ÞM'þ?ÙÅ~(Û?͏ÞM'þ?îìçYÑô?¶%ÚЊÌv?¡?1Šbà´?¶%ÚЊÌw?åð,GÆwª?µ¤NG™p^?Ô§ps¬?µ¤NG™p^?ïü®lîŸw?FaSCü?:Œ˜‹G;?FaSCö3FGL J1027.8+8253@_øA [À@@e¡"úÖËÀ:y¤O\_À<çCp˜?Ó»v«Ô/@
ܲ6žw¥@•¦_Р¿ã¼Ê}+¿Ùw£—–¬w¿å臿Û<÷"œô(UNASNonenone?ëD/Î×9Ý?È­·Fô?Âï@Ä£‰?È­·Fô?îɒ¿ÔG?¬	pÇi³?£fÔ¾kž?¬	pÇi³?í×(kœö-?¨´xO^ßÛ?±F¼£Nš?¨´xO^ßÚ?íw8ʬ?ª\gê%?·DF9¯¦?ª\gê%3FGL J1028.3-7419@rXú$‰LDÀ,=Žc|À9ê)€,À;X¸þ¹¯¿Ê›IÁƒÝ4@OFǏ¡@…:Ÿc2)¿ä¬Ú¼N¥U¿éÝ\0F]¡¿âHS‡Ö<|¿ïù۞ÕKTUNASNonenone?ïÕdgóóZ?€53D ?uMÌR?€53D ?êE3ÐRÁÝ?ʱª'…En?Æë0¾´ø‰?ʱª'…En?îq÷Oœ´Ÿ?›I¶ÉöÊÑ?¨à‹4¶
?›I¶ÉöÊÏ?ìwMQa¢ª?­üvæÍ.X?¼E•tòê§?­üvæÍ.Y3FGL J1030.0-5809@q҂ýuâ¿Ï¶™šróÀ9žü¯égÀ:H?³t63¿å­¯è)cj@Q>kµ±?ü­9~ÑÂ*?ã}M\¢¿æ_µj¿ç«®TÅ1ֿјšbŽ·áUNASNonenone?ßA¢<|…?Ðé'Øôل?à_.áÁù½?Ðé'Øôل?ëA
³Äó×?Ð2î`P?ÂûÕ0ì0¤?Ð2î`P?æ	ÙñAùX?´"|aa?ÓìL|
O?´"|aa?ïò$(Æå#?d˜S™¾?[·®r5¹¸?d˜S™½3FGL J1031.4-5855@qÛXâe,¿éôّmäÀ9/Q˜y*À:^2»>/?â,ù|rE@
­o‡l@®<_Å½?íc·yBP¿ÖËïΣ'¿ãPÊs^Ïø¿ÚY°~7UNASNonenone?êÖy"ÝøÕ?Áï¸z
‡]?Ħ°ˆ®?Áï¸z
‡]?åcy^?Ô`Í""}Ð?Õ×9
ôßE?Ô`Í""}Ð?éԙT˜wé?³KÄâé«?È­š­ž Y?³KÄâé«
?ë€X\Ú?¶]'?)Ñ?Áþžˆ˜?¶]'?)Ñ3FGL J1033.0-5945@qäîcŠ	¿öÃdٞlgÀ85׈±ÙÀ:k qäI?ᬜg`@
*l!à@	ohی¿Á žXùžð¿çe2´³%‡¿èK4ì=Lß¿ê­ò$'ÛUNASNonenone?¨HöŽ*x?³|ûsUâe?î{p—X?³|ûsUâf?¥óAo?µ¹ü{ñy?î Ï;éß?µ¹ü{ñx?ÕlÆÜíž?¸ÆþÚuìÞ?åIœó‰1?¸ÆþÚuìÞ?Ïoú8¶ñ?º)ÜÄ?è$1ÒD?º)ÜÄ3FGL J1033.4-5035@q›—Oß;@	U./¾4À9TãqT2À;_	ðCÊZ¿×QÏO!êû@¹ÿ´€¥­@'À
¼Ç¿ç³ÜæËQ¿ÕP¾Î M¿ÚLfó •ï¿á¸äÒAUNASNonenone?ïõ­YÆª?L¸gi8Î?T¥LÄr«Ý?L¸gi8×?𢡄,A€V?•)8"J"?…ôïŸê}?•)8"J"?ïzÐ\&©?‰…R9Š/u?¼eô{*Ù?‰…R9Š/u?ï΁Ž¬}K?pÞ¡áƒVå?x¿8©ÁZ¬?pÞ¡áƒVæ3FGL J1034.0-5731c@qÔ·éùr?âQ+6¯ÆÀ8‰Sԓj«À:m;Ì^èÄ?ñ7œvë¼@3Qƒ«E¾@D¨ƒñ?ïþoïÒ
y¿êBpI³—¿åMÞzýªÄ¿è´MŒÐ³aUNASNonenone0?Ýçu"äH?Ð[0b"²?á~E5Ü?Ð[0b"²?Ðß»UeW?љïWZ÷?çx¢UMU?љïWZ÷?ÙÀ…"⤾?ºi´!ñJJ?ã½5Ž­ ?ºi´!ñJJ?ÝY2
Þ?À¹¼¯+?áxôÓfù?À¹¼¯+3FGL J1036.4-4348@qjÚãæÄÆ@)9+6½+À:(ÇàÔÁŽÀ;²Y¥Ã£?Éx§À'›'@
‹+ÅUµ@6èßÒãè¿êbägYfµ¿Üõ>.þ‰ø¿Ñ2VG¿ïÿß¡ï1.UNASNonenone?èâ[\?д³oí¸Ù?Ï£§ˆv'"?д³oí¸Ù?ëÉÇ.½ö?Ç^KÄr?äØãE&?Ç^KÄr?åŽî_—É?ÆÌ2U×?Ôâ#@ÑÊo?ÆÌ2U×?ìD¨yt¬V?³='¹%ïÑ?½Ú¼4ZT?³='¹%ïÑ3FGL J1038.0-2425@p¿á2µ_@=;qdÇ)öÀ:29Úí!À;ÇÏ'ðßÒ¿ôtÞt"ý@PÓw`ߔ@,\@Gù¿çO•ßR¿ãlnÌ&J¿èøʕÿŸø¿ØFc]˞UNASNonenone?ïòŸÑy'"?cÉôÒ[?ZÀ]ú÷´?cÉôÒ[?ïÙʂÉv?}èîþ´
ä?s¾›|Å^?}èîþ´
å?ïAù²ò~?¥oÛ<·?—ÍàÉ¡°;?¥oÛ<·?ïþ6ØYn0?.JZ˜L<Ü?,'ziñ?.JZ˜L<²3FGL J1039.5+7324@`׆`ÔV@DG(àÉÙÓÀ:fK†ýÀ;éäwä=,¿÷æ©IåÒ,@ˆŸã	Ð
@À6 %#ü¿æ6…sO‹Œ¿ØŸ¹ÌÈx³¿á¤ºiÈƃ¿ãÍ
ñŸÿUNASNonenone?ïùuJVn?f±íÑ!?J*Ö¦EÁù?f±íÑ!?ï½3tV&?‹ÀÄ2#Þ?€³"êv{}?‹ÀÄ2#Þ?ï'ê…fCx?Œ8KœÖÌ?‹…^¦o!ô?Œ8KœÖÐ?ïþòJ4ª?%±nl?—^? Û\¶%^ø?%±nl?—Š3FGL J1040.5-5926c@qï™Ã‹«¿å¼^pÐÀ8À,ºs-õÀ:KŒÚw?ì/±>âúó@}Fößoè@U— E/_?ïÿÒ¯Kè¿çœ>˜ÍÔ¿è·ÚÙ8C¿édz"o!UNASNonenone5?Ü;˜'9Ë?×H2¤¶m2?áâ3·cv›?×H2¤¶m3?«_Ÿ\nÊb?»&Æêúk¨?îJ
9Z?»&Æêúk¨?Ð˹rÏl…?´D§èæk?çš#F˜I¼?´D§èæj?ȁc'½=}?¸( ÈÀ?éߧP°¡?¸( ÈÀ3FGL J1043.6-5930@qõ¢£Y6¿áʇ㎰2À8'oJ:¶µÀ:ɵÁ?ï¬çÁ½¡@˜ü§…ëg@†ü L{¯?ïïð`OËð?Ø{W­C£!¿â¯G›¿àõ°Ý)UNASNonenone?ގØìäUd?ϑ`-
~?ณ‰ÕN?ϑ`-
~?Ñ-¹K?üD?Ò7gÃô¨	?çi#Z`ß?Ò7gÃô¨	?ã€J5@¨?¶N"³‹™]?Øÿk•ñ~¯?¶N"³‹™]?Ùÿ˜üÔS!?Æb"^Ò0?ã3•Öp?Æb"^Ò/3FGL J1043.8-5851@qñDЩ*?Ÿ2±zƒKFÀ9qÁ
|À:¶,A§j=¿ãx×Ko®Ó@öôØ·›?þÒ_‡$!¿æÔ)9¬–n?ìS¤øûÝd¿éúvÚ¡X¿Þq'>|UNASNonenone?首MG?*?łôú"à?Ée¦ÊãV?łôú"à?èµå«­%¢?ÓvڤфÕ?Í(iQKi}?ÓvڤфÕ?èôî–'D?³Ô¨Ö¶ü?Ì,Gñ¥¶ô?³Ô¨Ö¶ü?ïR;Á"¿?œY+cCY?•¸‡ÍœH?œY+cCY3FGL J1045.3-6414@rIº^5À–§}‡ëÀ99ÀgmÍÀ;ú¶êã8?ôœÙ!™Ø¯@Ép륀@êvà1-Ÿ?î…а噿è5q—Ù[¿é°9é'BÜ¿í ¯"VU;UNASNonenone?´ H`¼˜Á?¸¤5kÜ¥?íköóèlè?¸¤5kÜ¥?ÄéÛü)@?Í¿|S5#'?ê'nõ¯û?Í¿|S5#'?Ó(;Æãʂ?¶TÔ:ËÀ?æk⎾?¶TÔ:ËÀ?ÂÐÍ[˜h?°ÔÑZjQã?ëK̾éæ?°ÔÑZjQã3FGL J1045.5-2335@pуùd@>à¼8*ùÀ:gK-û»ÎÀ;Æ¥®zÒ.¿ÑOƒ@r@
ö"»Á¸@ð¹@}ôx¿á»`…É$™¿ä½'J®¶¿çÈóœDnÅ¿åäS'¢FUNASNonenone?ïæp­u?p£ÜøCá?iíRŠîµ?p£ÜøCá?ïz¦íŸZ?˜¯1¤3øH?«=bLÅ?˜¯1¤3øH?î‹- ;C?œ+.ãÛ?§M&ýüKØ?œ+.ãÝ?ïRm¦ô_?‹V¥P`Ò?•²K!t?‹V¥P`Ò3FGL J1047.8-3737@qW8›R~@3Á;ŸÀ:#`m(!‡À;­ÓÞ9Û¿ÖܙAÃ;@¸
n˜å?þR}`}ï?»ÀÝf‰2¿Úœ91$T¿Ë¬šlu¿çi øÈÿ
UNASNonenone?ïñ™•ÎDß?_f"`3Ìs?\ÌÔcvAÆ?_f"`3Ìr?ïÌ01ã±É?'lëV¥n?yçç'ì?'lëV¥n?ï>F":G?' ‡QY-?˜7/x·?' ‡QY,?ïäÖ«Â?eZ"…‹ð?k)Tå€>Ë?eZ"…‹ò3FGL J1048.8-5006@qºQc4'¿@ <½ý&À9ýýQÏÖmÀ;pŽÉ[ÿ¿ÖyÐä½@
@¶
Í@cƒ 3Ï¿ëhÝûÚh¿Ó4IèE=¿ã2>^4"°¿êÏYVTíºUNASNonenone?íN‡àE+?²–ˆûN?µ‹ÃxýÖ®?²–ˆûN?ï%üÍL?ª-ãå(?ž@f^ö?ª-ãå(?ê$YÔq#?±"õ8A*?Çn˜¯ú;s?±"õ8A+?ï
·b3"?"O?Gi²T?žI¹ŽM"?"O?Gi²T3FGL J1049.7+1548@luâlv@MÎ#žj¹²À:Ë*5]°À;Ò·£oÜ1?¹'ÄD©Wq@DÄyl'›@9Qx Ñ¿ÇD£¼ãýV2ø¶ò¿Ùô"U~{u¿íCWŒšUNASNonenone?îö†9¸Ó?³g)Tô'?® —œdrÑ?³g)Tô'?îï÷–'fP?¢DaÍ ª?¡†‰›?¢DaÍ ª?ë&ƒÜo4?°æÃÂ??ÃeðÂC1?°æÃÂ??îÏ ñO{?˜SsΆÜÄ?£ÿëW?˜SsΆÜÄ3FGL J1050.4+0435@n±
gb@J´Ø]ú‡À8ê'"ÂÀÀ;s˜~§?ð%²úh¼W@ªð†y@ÂÆ ‹:Ü¿äæ}MŜ¿åmÏ557¿é¾Š¥ñþ¿èéM¯VUNASNonenone?ïüiÀT?@êg5ê%ö??±ÿÝcp?@êg5ê%í?ï»è¤`Oö?(Àû±ô?ÖçìC?(Àû±ô?ï="½&&˜?ÝxÅ€/?˜Oh[;-?ÝxÅ€0?ïó¤+$"?SÕBðÆÑÔ?X·ÿ©¶Öo?SÕBðÆÑÒ3FGL J1050.6-6112@r {5*"¿ú¹ýl§ÉÀ9gâTÀ:"Ö)làÔ?ñ^¦ß'mW@
á>µ[E@Ñ.à=B?ïþò7Y¿ëç…* åÔ¿ïÿí›ði?ïþ¾M¥UNASNonenone?çàU×j{œ?ÒR¼ Ã´?Ð?TQ+É?ÒR¼ Ã´?çt)×G?ӈJK—¼?ÑÝݬQs?ӈJK—¼?á;ÍñMw?¶íäíï&?݈dée?¶íäíï&?ë­ºóVçî?ÆÞß.O‰?ÁI2¤`M?ÆÞß.O‰3FGL J1051.0+5332@cUŁo@KÁÆ*\}À:{ˆe"¯OÀ<ñ¨Nh¿Î%+Ž@™ÿ¯Î@﹞¿ëvTÀ*æ¿áº—âÏ}¿ïÿ)Î'V¿ÜZN>–,–UNASNonenone?ïæŠéW5?|Ë_0¡5?iu¨çËp?|Ë_0¡5?ïòÒKP¾?«('Uø?ž!¥¶•è&?«('Uø?î)ž»šd?¤²¸Qͅô?­fF^É­?¤²¸Qͅô?ïSZÔ/?'Z_u¨?•"¥zÁ?'Z_u¨3FGL J1052.0+0816@n!ßzNz·@Lr)ZlÀ:{¨G²F9À;ã!"Î~~¿¦FéC\~@Í\%DÞ@ÉÇÿÞr¿ØçJÿz'¿è¤¢P¿åGrI7p¿´ÃÂV	¡UNASNonenone?ï—Ì/$?–~ÂI_ä6?Š=Ìü46ü?–~ÂI_ä5?ïO)Ö¼¯¨?¤GÕs9F%?–Å(j?¤GÕs9F%?í#ëÍT>?®lÊU"éî?¶à¡•_Ž?®lÊU"éî?ï€ä¶ö	?‰®'ÒEjr?ÆÒB|ýž?‰®'ÒEjr3FGL J1054.2-3123@q7KƧïž@9'¹¾ÓÀ9ëUmßÀ;³'ìüíý?ëçBXÑ9@h|	泩@ÀÚñŒö¿ãFBÂGbÀ¿ëSVÞÖ\¿ç҆²X¤©¿ïþçSá©~UNASNonenone?ïè,Æ­²?jS5«Íښ?gpÓ9RM¥?jS5«Íژ?ìæKY#ñs?·ièqt?¸Í¥6àth?·ièqt?íµ&þ7[®?¤ŒA٘1M?²VÈE""?¤ŒA٘1M?ã÷ʺi?·=@ÞÙð?ÙÖüj‹-?·=@ÞÙð3FGL J1054.7-6006@r
£Âˆ¿Ý'l¡"ãøÀ8…æ<à[À:7 Wù¼?æ¿M:ö@
Æ`Â7{@i³ +9?ï÷‡'að>¿êò1¡°¿å±ÊsbοáÉZ
§<´UNASNonenone?Ú.M	¼b?эfa÷Ø?âèÙ{!Îö?эfa÷Ø?ܪ"ÄSŽ?ÔÀfWz³m?áªîüÖ9?ÔÀfWz³m?à.'¿)…æ?½ÓUò{
{?ߢځ¬ô5?½ÓUò{
|?æÈVòö-o?ÃhK¯ºã|?ÒoR¥%?ÃhK¯ºã|3FGL J1057.6-4051@qŒ¨$x@1ÙUmÀ:yߙX+:À;Äîð
Cµ?äQSzW#@
êÖxF?ü#Ÿ—_ƒ¿ç	­³ø¿âkrÐé"T¿¿}t$¿þ¿ÁÁZà˜¨ûUNASNonenone?ïï¢L1ð?aÝé"‹?`]³ÎîÓ?aÝé"Ž?ïκƒÙ}q?ƒ|5'°g?x¢¾AG?ƒ|5'°g?ïsrNf';?ˆ=
>Gá?''¶3/¸?ˆ=
>Gß?ïx\ï|"¾?Š$ºøƍœ?ôbmh*?Š$ºøƍœ3FGL J1057.7-6624@r>1[W>«À}'ÔÀ9«'!üÀ;<©Ôz@?Éþ"7ëÝ<@.®oês§@­-êñÑ¿ãG=Çå:¿êÌj¯ÔÌÿ¿Ö—¿s5W¿âÛמ%ß'UNASNonenone?ï¤XðކW?™ ûÇV?†éÃÈ^j.?™ ûÇV?ègpځ?Ñ|
åÀL?Ïîb?Œ•ú?Ñ|
åÀL?íVšU3á?§'û ù?µK-Vgô?§'û ù?éÝ}R@›?·;eöè?ȋŽ
¶ý–?·;eöè3FGL J1058.5-6106c@rœwškQ¿ò¨´wkÀ9&5îþÀ:HDK‰kN?ô—–"×h@E¬5¨ƒl@BÁf½y¿çZÙÀ¿ëûÑD¿ÝAåu´œ¿â_¥&À‰UNASNonenone0?Ú$iü¸¬¾?ή°ývç?âíË£©¡?ή°ývç?Û隇'½p?ԎÍÆÀp"?â2¼>¡H?ԎÍÆÀp"?â"à‹ð'?¶vÄ-ÜÉì?Ûº>èôÝ?¶vÄ-ÜÉì?ãZ?m?Æz³× y)?ÙK%ûÊ?Æz³× y)3FGL J1059.3+0224@oY4Â@Jį¢ðZqÀ9˜ô¯úÀ;L"ø?Ûh_¤D1L@ªæÂAX@ÐßÀ‹¿´1]¥Í"ƒ¿ä¬ùAc¼W¿æÂ!=ƒ`¿é§"ü»kÀUNASNonenone?îu!I½^ò?°bBõ6W7?¨­ëd*ô?°bBõ6W7?îÑ¢Î)?ªàŠÓaå?§åÓo?ªàŠÓaå?é"3ýht?³7N"›ï…?Éï0
^/¦?³7N"›ï…?ë<ÌÖÌ"Æ?¬éT4q
Ì?Ã̤Ïtì?¬éT4q
Ë3FGL J1100.2-2044@pë•a'@A‰°¢ÊšÃÀ:H–ÂNĉÀ;Öu¼D¿M¿ï-Y[ÇO@þ\¿sÜ@MÅ¿g^‰¿íF½K¿É€tR8S¿ëA¤4Óp¿ÜdÌFÚUNASNonenone?ï¥pÄ:ô€?'+B Ò?†£ÎñBà?'+B Ò?ïɃjæâ\?'ÇrR¡[?{>JŒŽÒ0?'ÇrR¡\?îf]ÃÜÁ? 0r,¬´Å?©š#΢3û? 0r,¬´Æ?ïô{ש7?VÛûx?WP­'ËÏ?VÛûx3FGL J1101.3-6032@r²-V¿àS.øî¿À94íbnŠ!À:lÞÁÁÖпÓØe—^€ê@
°Øù‡Á?ÿu˾Úƶ?ïá…ï¡@¶¿éᖸ52‰¿âV?Zf†¿ça
˜¥UNASNonenone?ïj<ƒþÿ?›çÑ
™…?'¸/€ 
?›çÑ
™†?è1Vˆýµ?ӋF=ŒÖÙ?Ï:§¥Ü	+?ӋF=ŒÖØ?êš_nv<?°`ùÈw~ô?Ŗ'Eú'?°`ùÈw~õ?ïr¬{ÊÀ3?—6p?'ªp†§ù›?—6p3FGL J1103.3+5239@c93Úøßz@LÀ!ÀD(NÀ:At™/À<¼²£V¿¿iòC÷%@µMBs@ñç_u0"¿à"°¦Ùý¿ê-	ﻐ¿åSÅÀÐ%ƒ¿ïþ'ÝQn!UNASNonenone?ïúp1¬{?^µ4k?F?9MÂ?^µ4k?•6LÐ?«Ýrùí/?¤F欛2ø?«Ýrùí0?îñRFÞàÏ?—1Ýßâ7? êےó?—1Ýßâ7'?îß­Á{''?™""µý ?¢#èF݇?™""µý 3FGL J1104.3-7736c@r'—CécÜÀ/é‰XÙµéÀ9ul¡
ŸÀ;Qý¢W®=?ïd»þ8@O¥ 
Œv@_y5¿Ôpͼ¥§¿éM­TXê¿å_Xœ"ü¿ïÿGã<¦UNASNonenone!?èö`2°J??ę3¢/ÈO?Ì&5>×?ę3¢/ÈO?Þ¸ù›Ò…?Ñ•ž--?à£÷2¼?Ñ•ž-,?䨷»Yƒ?·¸¬Ü0ˆ?Ö®‰ÕLù?·¸¬Ü0ˆ?Õ"jµµ®?¯\=q>2?åxµÊ¥%)?¯\=q>23FGL J1105.7+4427@dÕô!-w@OSS&ÂÀ:Ž=EíÀ<;tÈ)¿³"š²@
Îò+Öó@>Û_· –¿ã[ºæÆH¿æqrð§6T¿ä,OÖÏQ"¿à}J$þUNASNonenone?ïFȶ)®?°œcûÎ?—&üÉ:ÊL?°œcûÎ?íüƒv'8?¼Ct$ðÀ´?°äKk†??¼Ct$ðÀ´?íøp ‹î?­X‰
Í!?°?,zû ?­X‰
Í?ëZ|¾G?·ÍîŸ÷ëe?—–ýå?·ÍîŸ÷ëe3FGL J1106.6-1744@pçquŽ!–@C7-À:BHû"±À;¿~6fÄZ?õòs´@
2"a¤
@Bÿ¢7"?îmÇÆJ)¿Ð÷–±Õ¿ádZäªm¿ïäÈQ'ÃUNASNonenone?²×e ó?ºÜ6¿×‰L?í¿EKáž?ºÜ6¿×‰L?¬éðûW?¶tl½Ü>¹?î>Q`ðGê?¶tl½Ü>¹?¿áù³áã?°Š¸wEX?ìÀɝ£Ã?°Š¸wEX?¹¢¦]W"*?§ë=…ï%?ìË«4U
{?§ë=…ï$3FGL J1112.1+0500@orÓEŒÒ@LÎéd8À:T…òó¨À;À°',ãŽÀç§íå@:jôºL@¾ó ¡Ë?êÿßfWwá¿âóq@"õ¿èj~‹¿ÍRU`7UàUNASNonenone?ïÕ}O¨eü?'áÅ;ÊÝ?uAX+Í?'áÅ;ÊÜ?ïÐH›Ì?‡îQO{%l?wÛ²xý½?‡îQO{%l?ísøoŸ"?ªÈ¬éá ?´`?tƒd?ªÈ¬éá ?ïÿü!ȇ7>Ðñæ€3i8>¾ñ»ÆHzƒ>Ðñæ€3i3FGL J1112.1+1034@noY_í¦a@N¯hð"aúÀ:TËf›@À;Ë
Yö›¿´® HC@
ÙùXqQ@á'À8iÔ¿åK/99‰¿ì}0ÂÀ"j¿éÊãÙâ<©?áb$•ê;UNASNonenone?ïøÀGxт?S׋ôlç?Lþâ¹õº?S׋ôlç ?ïÀ.X%ù}?‰y_ï¬w¨?èÓíAÁ?‰y_ï¬w§?îíÂѨyÙ?—ÛE?¡#Òåxbo?—ÛD?ïïûfæN?cZ•ÿ‹ˆÁ?`ý™±ú?cZ•ÿ‹ˆÁ3FGL J1113.1-4515@qÕ¢£Y6@,z2	g‡ÏÀ:)ÆäUŽÀ;†N']‹?Í
Gö'¨Õ@
§ÍÓËD@–«ß—TÆ¿è2Ùhˆ÷Ø¿âÏnhF¿äT®€¨Ô¿å7&@l½ÕUNASNonenone?¾7,š?¬èŽ
Hú?¥¶6f?¬èŽ
Hú?ï0"i°yS?¥WOÃ>'Q?™ïrÉðՖ?¥WOÃ>'R?îDcÿ¿ã?¢}ìà#üx?«¹ÀÎJ?¢}ìà#üw?ìÑG>¼ñ?¨áæÀr=?¹uÆ
wé?¨áæÀr<3FGL J1115.0-0701@p'Â;yRÒ@HQt>–=ÅÀ9²!gXÔ­À;¥¥
æãÏÀóEâ¸Fƒ@ÛÄÞ@è~@ÞR 3Q;¿â¥ç*úˆ%¿äʑ5òÖ!¿ÛH´ª>†¿â§¡²AÜUNASNonenone?ïÿïÿî~Ý>Ý)®íã0>à";½>Ý)®íÙ?ïÃ#`6®¤?TÖ*‡!?~nO䨮J?TÖ*‡!?ïëÎÑߨ?p:éýb?d1. Wé"?p:éýb?ïÿþ¶$œ>¸í
Ú\€Ç>¤žm¶FÑ>¸í
Ú\Œ?3FGL J1116.7-4854@qõ>"åÞ@&)÷LsÀ9ÑûÊçÀ;veŒKÓ=?壪¬2ð»@—k0O©@­J 4¨Ô¿ã°ÝŒ§\•¿ç·ó…âòB¿ê&µ×›e¿á³
¶w½UNASNonenone?ïïéÅÅ?e0ŠËÑFm?`ñç:;
?e0ŠËÑFm?ïAÝálŸB?©5}U?—ÄCÒlã?©5}U?ï"Àî?"패å~?›½<çþ'=?"패å}?í'lÿI?¥×£ "?¶ÄŸh³?¥×£ "3FGL J1117.2-5338@r,\ý
@¸èBt×À9_Çȁ
²À;aHZ⤥?ϟNéÆO@Ô>¢ýñ]@uÿ‹í¿å2. ­R<¿Ü<
"¦¿ÓÒ×CÚ['¿â]֘[3¶UNASNonenone?ïýœ*°(R?1ÐËÞ¥_J?3ª~½v%?1ÐËÞ¥_J?ïµ;ê ¿u?'ÅvCÞ{r?'±WÐ"¬?'ÅvCÞ{r?ï½ã×ô1?€Zûâ3)?€‡:Jóª?€Zûâ3%?ïÑaf'•-?ic!©˜E?wOLì5iÛ?ic!©˜B3FGL J1117.7+0217@p
Ô`ªdÃ@LDêòRÀ:0ªRNmÀ;ʤŠŽcÛ?××2lõÝÎ@îáI±z@9è_ÐJ0¿ÂOØÊã¿äÙGdÌ¿ä"ùiÓÈ¿ßþA†TÇUNASNonenone?ïò"j¤eX?fË)X?Z÷*·5O?fË)X?ïˆ]"Í?"®²TŠr?è¸Û:LÚ?"®²TŠr?îøŒRté¤?˜›ðC	\-? w:رeÌ?˜›ðC	\-?ï)•w¶1?Ü™±Ú?ZÍQ	9ä?Ü™±Ú3FGL J1119.8-2647@qmMüã@?ÂÚ/­mÀ:j<?KojÀ;ñÅ	‰ì¿ÆÔ_ï @ì;›ât)?ýSwê"¿í\B_[ö¿æ&+7]±®?ÙûHñÓ¿ãZG'öjUNASNonenone?ïÿb¯¦'?9"Ja͛?¼ê-Ïv?9"Ja͕?ïÑ뜆m?G¢{¶7?w
±¼Éh?G¢{¶6?ïázS^Ä?r.Y ÁD?n…¬ñ¡<¶?r.Y ÁE?ïûEÊõös?Qy3çD?BèÔ(&3\?Qy3çG3FGL J1123.3-2529@qpö@c^@@¡˜¿pÀ:$€èȬÀ;ȯf•¿«¬"'µþ@kÚÔ¢Y1@Líõ®˜?ë+Uæïì¿çÙi‰9²¿Ø΂‰ÝŽç¿éxuäw})UNASNonenone?ïÚ:FNÅ?'ñÑ%4"?râø\؞d?'ñÑ%4"?ï=?"ÙBd?žüárP=ó?˜X
d׳Y?žüárP=ó?î
a&¥âÏ?¡
Üöøê?¯Y핡Ó?¡
Üöøê?ï¤F[Û?•‹ä|¦?Ÿ|kw4" ?•‹ä|§3FGL J1123.6-4558@qö5ü;Oa@,y‰7KƨÀ:1íÚcŽEÀ;šsîå%‰¿mYñäv‰@º\JØw@Žc|?ïýFýå¿à¹f™ù!%¿ë\D¸Ü³?°â×Ö¢*æUNASNonenone?ïÎv²fø—?ƒ82ЭGç?xĦ̃´î?ƒ82ЭGç?ﳤÄ›4?†´ÃV˜|?ƒÎþÙ3?†´ÃV˜|?ìn¯!{?®Žõ04Î÷?¼‰ïʆô#?®Žõ04Î÷?ï,Ü[Ù1³?˜ˆ«w?šdt"ÙÉ ?˜ˆ«w3FGL J1125.1-5803@r;N…3±@S¼Œã©À:RT`ªeÀ;9,G†§O?åu5¯—æD@
↏-?þw€?*¿ïìꏈý?ä<aëyÙ?™©¤/ó¿ÜêUU¿FŸUNASNonenone?ï¿ñ¬.Rð?ƒn››f_?€"ôkD(?ƒn››f`?8.ë´?¶ÕX؁þ©?¦¤¼}Dº?¶ÕX؁þ©?ï³"A?'[\œ?œÎ^iwä?'[\œ?îZQì[?¦ò••4?ª^šá:OÑ?¦ò••43FGL J1126.8-5001@rҝÇ%Ä@%1uÀv}5À9¢V[LÀ;Œ•ÚÈ8?â£ë#î^@
 úS˜®b@ht`O $¿èµBÙ¿àÑ3cښì¿èAÌsê2¿é¨ó8hɏUNASNonenone?ãú6Bj?Í)³öÑ*ø?Ùß"{+?Í)³öÑ*ø?çhÙUÎʏ?ÏÛÃOðRµ?Ñ.MTbjß?ÏÛÃOðRµ?èÔ֑ÚÖÏ?´Ó[*7‡Ü?̬¥¸"¤Á?´Ó[*7‡Û?àÌó›¦tò?¸xi%Êê?Þfȳ?¸xi%Êê3FGL J1129.0+3758@eõ5¨Xy>@Qf&,ºs.À9€E¯6¹ÐÀ;|išÎM?î6oùÀ©\@h¬¯Kº@N•`Nõ1¿·ÇúË¥À¿äÑ/÷®<¿áú6Æv؋¿ìuƼEÊUNASNonenone?Ôk>9¦ž?ˇ\FÛÓf?åÊ`ãt¬±?ˇ\FÛÓf?åG¨?ÏÛ5Ã0?ÕÐáqá°?ÏÛ5Ã0?Û>c'h¡?ÀF݊½Þ?â`ñN6˯?ÀF݊½Þ?ÕB ¯cÜ?´Æzlq
?å^ÿ¯¨N?´Æzlq
3FGL J1130.7-7800@rª"záG®À/ 0 ±»ÏÀ9è<ʋ©íÀ;ƒÀü´ñå?ëe-žÉ¯6@½~Õ(Z?ûØ€nz\¿ï±Â¦"e?åv´@;¿¥šŒéÊîØ¿ÒùHápGçUNASNonenone?ïÆë™4°/?|'gžêµ?|Š3e§èŒ?|'gžê´?ï‡Áwìl? (haB‰?Ž¢üå? (haB‰?îÉ—ü?–;R}ŸÏˆ?£o–Žà>e?–;R}ŸÏˆ?…#¾?›àoÿm?¤®†'­Ä?›àoÿm3FGL J1132.0-4736@rZ¬1@*SQÞïåÀ: @‹áJÀ;´)Žnÿãê*ÍB>@±§+'¡@韍#•¿ïþž-Ò÷?ïÝ[Qy36¿à¬¤±®@ù¿æ3²UìàWUNASNonenone?ïùËíäÒ!?I¯ø:¶/?HÐHl·}¤?I¯ø:¶+?î‹ ¬)›?³S–¶ý§?§Mõ=fH?³S–¶ý§?ï…ñÄ°	?… ô\2?ŽƒŽÓý¿{?… ô\4?ï(*µÅd®?›zHã ?šú©GSjL?›zHã 3FGL J1139.0-6244@rkî¢	ª¤¿ðZ*~…À8%ô¬å§À:…"_u±]?íä+¬3ب@·õ$YÒ@2^ÿê±d¿ÜSä,©›¿â$ËdÓûP¿ã1O¬Té¿êc€ò†UNASNonenone?¯ÇV¦c¾?±}Éäyt?îŽ:•™Å?±}Éäyt?g½öÂˆ'?€xÝ5f?ïèB	~=w?€xÝ5f?Ï7A]¼Ù×?¶ÊÆ:üÞ¢?è2/¨ÉŠ?¶ÊÆ:üÞ¡?° ™c(ìû?žæ€½
(?íëìӚâ`?žæ€½
(3FGL J1142.1-6941@r\|ؙÀ}¾Ý 'À9¾±û.·À;:Æ/#Ú¿Ú®ÛÌ*K¿@ÝX›L¢@F˜ÿÀ¿ù¿ÝnŸ+:&©¿è槍çÎu¿è(Aš Ÿ¿èŸÈ,¨LUNASNonenone?ïåó̂¸?p¼«Xg›?j3}ïH¦?p¼«Xgš?ï_ùƒC
?©˜‡àæ?tϗž¸?©˜‡àæ?í©ÆºI^Ã?¢$™²(œ?²±Ê-µ	í?¢$™²(œ?ïÁƒ¤"H°?t0B7ݎ?>-µÛ§Ä?t0B7ݎ3FGL J1146.1-0640@q8Œ½D¦@JWe<š»À:EFšï/À;¼ì÷À?å×r%?Z@éeß­Ð?þ»È?õ8|¿îZÖ×"ø9?ÉxLÞ¼»¿Èܸûè ï¿å 5j%UNASNonenone?ïâìÑ Õç?nL(ÈÌó|?m.ß*ß?nL(ÈÌóx?ë°ÊwË°?ÀÑwFÐÃ?Á<Ö Ó™??ÀÑwFÐÃ?ï7L½þW\?a!Ÿt?™h@5x?a!Ÿt?è>¡­ÅFî?ºÇˆ"yñ?ÏyHêäH?ºÇˆ"yñ3FGL J1149.1+2815@i•nÖwpz@S¤i×4/À:JÊ<ϔ'À;Ï#K^£$¿ÎþŽ]GÑ@¨¹ù¶dÖ@©¶àQcö¿ëÂ`?äO¿ã~œbC8†¿ÞôRds>ˆ¿ä®àc隟UNASNonenone?ïù¨ŠóÀ ?YÀÄ 	\?I]Ô0ý?YÀÄ 	\?ïvLªäû?¢ª-Jú­æ?'<Öj£`œ?¢ª-Jú­æ?ïKòVҗL?"¯ù¬Dõ(?–µ%­ƒ?"¯ù¬Dõ&?.y¥,?‡/Ûëk5?Ž]ôa–´ñ?‡/Ûëk43FGL J1150.7-4816@rIø -à@*½½×fƒÃÀ:Xóz¶ƒÀ;¼ AS‡g¿Â
ÎʨÛ+@ùÔLfá@¢ÿZcN?Üù)Ƒ¹¿åՍÌÂø¿ìÛ·ÿ¾Å+¿¹Œoôág.UNASNonenone?ï·Ǚ?¤"íoE§?œé§މ?¤"íoE§?ï'ái¢ú´?¡NW(í4?‹G¥—AS?¡NW(í4?ëʉbT?±í€¹å{²?À×½ÚuŠ°?±í€¹å{²?îôÑJRÅ?œ¸<üJÊ? ²ïÛZÓÁ?œ¸<üJÊ3FGL J1151.5+0957@pJ^~¥øM@PñŠÚ¹õZÀ:|ـ9vCÀ;âÍ)Á¿ö­sU¸`@¾_ ø@Ŝ@Ô¿ßےêË1ä¿æ)jÀúAá¿Ü¡ú¤t¿è‰¼qOUNASNonenone?ïþqF?6ª$•i}?/×(ï»®L?6ª$•ie?ï·-6'ËÉ?':´<d?'4²v

ò?':´<d?îÓ%Á'Õ¢?™s¬@'…ˆ?¢Í£í'¥Û?™s¬@'…Š?ïù¢ƒëuè?P¥
ëáŠö?IuðR(]˜?P¥
ëáŠù3FGL J1151.8-6108@r|Щ*0?ìʏ۪¶"À9	ï]ñLßÀ:ÒFfޏ?êZz%q9å@ðé‡B©ô@w†ß­¥¿Û?€UrD¸¿¯;!îV#<¿ë#Â2G®s¿íÔەx³×UNASNonenone?"'Ö:OFº?')ø c4?ï­¸§Âä?')ø c4?®¯¨O¤±=?¼ŠÖŽϜ?î{´ì?¼ŠÖŽϜ?ϗ,˜?¶a'Û…¨?è4Ùø~y?¶a'Û…¨~?ÓŖèüŽì?ºÚϼÏ
?æ4‹¸Š?ºÚϼÏ3FGL J1155.3-1112@q˜|ßýa@H©>¢Òþ?À:ŽK†ýÀ;£1ßÈR?ð
ƒ® ¼Î@`þWN?øIúÑÃ?é#ÛΌ.f?ëšG>'ó?ç(fº¿ß/DÜRü§UNASNonenone?ï¡Â†ewN?Žç¢B?‡^f¢,¾?Žç¢B?îi%=¯¾?¿Lò«A?©m¬%Ó?¿Lò«A?ímíÕʒç?£ì"éo§?´'Q«hÉ?£ì"éo§?îâÊ.õg;?²_á<®‡ý?¡Ó]©ŒG?²_á<®‡ý3FGL J1200.4+0202@q-¼U†D@Oq²•êÀ9ã£v'-•À;¸îA'šÈ?ß	袧pƒ@#æ9/w@H½§Õò¿çEÂ[H"Þ¿Õv.­3÷¡¿Ôc)ÖÖ2¿ç¼*¥ðêäUNASNonenone?ïæÔ%ñ=?nŠÁ"¾?io+ÚÁü?nŠÁ"¾?ï8÷O¿ý¯?}ÆåSå?˜áJ1?}ÆåSå?ïfj a|n?žƒí?"2»óÐrC?žƒí
?íî38" ^? ˆê£' ?°Žf;fý? ˆê£' 3FGL J1200.9-1432@qÐVÕϪÎ@GHw…À:NÌ7«hÀ;¶­¦–Ø?Ãwx'7ûo@ø,*€\1@)«0ñ¿íŽä["ª>¿ÜI6¶† ¿ÎßÎÅ~–¿âVÎÜz"UNASNonenone?ï÷+ ãYÓ?WÇÂÝ?Q©¾9LY?WÇÂ×?ï‹dƒ'5?˜,U5Õj:?&ÿßr©?˜,U5Õj<?ïWÙ;ƒ?š*æ«l™?ŸÕ؝o…?š*æ«lš?ïÅÖÒ8rå?t!é³kÊ?}–ãƍ‰?t!é³kË3FGL J1203.9-1745@qó\=îx@EÓÊ}g3ìÀ:R·*¤yÀ;ק jٓ?éð¸Á^ã@ù½',±@ZH@5¥(?ág6s|¿Ï¡ò3Â-¿âýÕÊ2¤Ô¿ïÿ'wJUNASNonenone?ãAÃ'î"?Е`ëô‰—?Ù|yÆÚ#¼?Е`ëô‰—?Û/$†P 9?Ïl¿a9ê"?âhm¼×¯ã?Ïl¿a9ê"?ãþw5k;î?»{dlu¤–?Ø•)ˆ&?»{dlu¤–?ßHPg1¶ä?¼êo±kh?à[×Ìg$Ž?¼êo±ki3FGL J1205.9+3315@fGohی@S›Då^³À:WÌ¥_ À;èÚ'QU?ä¿ÃôOâZ@
þƯâÜ@·9_‰¿íøÔÔy@¿ÞòÇK;¿äÕxÔ
o¿Óý™üÉrXUNASNonenone?ï3µ=ቖ?¥† éöu?™‰XCÎÍV?¥† éöu?ï9ª½s!8?«W´kd?˜Ê¨Q›Øñ?«W´kd?í±MžWyè?¥4è
ûò?²u"
D0¼?¥4è
ûñ?ëF}ÙÓ?·áŠ–êl¥?Âæܘ³Å?·áŠ–êl¥3FGL J1206.4-7123@rµ7KƧðÀ!®ªm&tÀ9ƒ@ìYZÀ;k8$3»ï?ê'~~@%¤ÝD"/@qM éÀ¿è'½{ºÐ:¿é8úž}jJ¿åÚ´¼Dñ¿ïÿ¹ý£jUNASNonenone	?ìí:¹
p?¹y×ȯè?¸–/7¬?¹y×ȯé?Ë'íˆHÂ÷?ËzE45ÈP?é6íÏC?ËzE45ÈQ?èÝ+Þg·?±ÿc¹g(?̋SІa#?±ÿc¹g(?Ð÷µù¿Qˆ?±¼3K!£w?ç"% W<?±¼3K!£w3FGL J1208.0-6901@r°µ^ñýßÀíäßé	CÀ9Úe;ÃûÀ;hK!f'?ç'͌\½@
¾öJt˜@ÞÛÿo·H¿ç¦2™°?οã/žùÅ¿åÙx(¨F¿ïÿíK¥ùWUNASNonenone?ß8' JÝç?Ðch
ÃÇ6?àc¾ïڑ?Ðch
ÃÇ7?º9,"ZL?Áõá"΀?ì¸Ú{½¶?Áõá"΀?åªzàÎ+ª?µJx"þmâ?Ô«
>c¨«?µJx"þmâ?Ë*kÒä?°ÁāA~?é5e=}Ç?°ÁāA~3FGL J1209.9+7607@_Œìk΅4@D^™côÏÀ:J¹¥¨œÀ<{DD¿Ó4ƒÄ‰öþ@
§ÑjÁ?@/`œwð¿å–âcâÓ¿èësg<¿Ñ'Û ïÜ¿í>vÒçjUNASNonenone?î—ØG‰x`?µÁD#e?¦'{‡hyô?µÁD#e?î¢í~'5D?¨VKýÑ1?¥Ñ(Ü«¾?¨VKýÑ1?í/ª‡ùÅ=?¬Þàpï(?¶'«À1Ö?¬Þàpï(?ïwӖÖEÕ?‰ÂE&+E?'%7Eh?‰ÂE&+F3FGL J1210.1-2742@r>ýuâ@A"–'§\ÑÀ9©±¿*À;€8YáÀÔ7cnU@ë&šž|W@¾Ç :ˆ¿ç­U™c¿ê]hÓþð6¿ØR×	Þób¿êà‡Q:UNASNonenone?ïÿå&>ìdÉùIÇ>êÙríä)o>ìdÉùIƒX?ïØ#Iý-…?5Lȶ?sî[i=Æ?5LÈ·?ïÎöL
yó?~"Ü`éS?x"ÙúÇ?~"Ü`éO?ïÿü²v^>Ìöo¿Åô>ºlM'_>Ìöo¿ÅúÈ3FGL J1211.8+6413@`>ŒSâÖ@J.VCæÀ:Ì-–;@HÀ<3¢¾‰­¿–Ü,ïªÑ@
%›@xqû¿í¶âyÔ¤ª¿ÉƒËÒ{¿æُŒê"¿ÜœVH9UNASNonenone?쾂Ío›?Â[Чx:?º锃#}?Â[Чx:?î™{	NZõ?±"±1 >¢?¦hOkP®?±"±1 >¢?ìGQÓ¦^Ö?±nld ?½ÅqbÍ	L?±nld ?î=ÒôŚ? A78ýU?¨"г¦Z? A78ýU3FGL J1213.9-4412@r~Â&€@2$Wâ?$ÙÀ9›Õ¹ÛÀ;"«² Ñœ?¤63©åv@üW-
E@'§_ÕӇ¿Öaé0¨
î¿æázéÞ´¿àsHš(½¿é}œ/mxUNASNonenone?ïڄ1Ҍ¬?x±AÚø?r½ç¹©Å?x±AÚö?ïuvjìëå?"èÁ"Bœ?'Q2¢bƒH?"èÁ"Bœ?íæCe—Œ'?¢q°FH*?°ÍäÓCžÒ?¢q°FH*?îÃÙrÕÃ?'Ù¸t%Ï]?£ÂhÒ¯óç?'Ù¸t%Ï]3FGL J1214.4-2315@r?÷eýŠÛ@Ci/Âej¾À9õÅGMƒÀ;šñ,'¦7¿ÝöECM@

ÛF["@‡Ÿœ¿äšgãq²}¿ç¨ýÀ	ÅÒ¿âB`m†žÉ¿à5\ë_×MUNASNonenone?ïüw¬Ï¼?@dñ"‰?<B™‡\?@dñ"Â…?ï([b)}É?§F]ŒÿÜ-?šô"ºÐFì?§F]ŒÿÜ-?ïmX·£ ?Œ·ˆ|?'Té‹ý€?Œ·ˆ|™?ïŠ÷äc¦?†›qÙå‰b?B8Æç'?†›qÙå‰b3FGL J1215.9-1926@r8Œ?>q@ES3"l;'À:-H*;<íÀ;ºêßÝJÉÀaa;.T@—ÿÀ@Pwߊ"™¿éßv\›¿ãñ¨‹Üë¿Û€Sɱ¿í;=ž¤£ìUNASNonenone?îtňeŸÇ?ªÅ¨Ç|*?¨³§y¦?ªÅ¨Ç|*?ï"ö!?£>_û†&?‹88Âw¸'?£>_û†&?ìRñ˜O{?°Aºöô°ô?½hw3="+?°Aºöô°ô?ïÿ0¡z|?/|¶!Œ'?ý«Ð°'©?/|¶!Œú3FGL J1216.6-0557@qö8<òϖ@Kí@$³=°À:o®
ÅÀ;—\>Å7­?Í,Xæ˜ð@ü;û-Þ@Ý0ŸÚü:¿ç½žÁ¡ y¿ä°ÎøSÁÒ¿ãu7	àC¿ïýÌn®'UNASNonenone?ïìú<Í?ƒ_ðÿ?cüÃb3	?ƒ_ðÿ?î|÷HÉ4?«÷rǹ3?¨0‹sl¿¬?«÷rǹ3?îUó6*δ?Ÿ‡;ã׃å?ª ÌS²?Ÿ‡;ã׃ä?ìòÅ`NÂ?¨]äŒÀû?¸iÔý‰ïX?¨]äŒÀú3FGL J1220.0-2502@r_ÍÓØ@B¤!ÀD(NÀ:WfÛl7À;¬—AЄ迶
ˆnÚñV@ŠJ}Qº]@r`Æ%¿ïÆ»y$?ÜÎk6Ʉˆ¿è>)YÉ(¿ÒÈ*Ïj£UNASNonenone?ïÔ÷ÁYo-?z…Cà°4r?u"SHiW?z…Cà°4p?ïºxdÖÜ?‡	dS•M?aæÊzˆÖ?‡	dS•M?î"Ày9ë?Ÿ5ff+È?¦³ølaOä?Ÿ5ff+È?K½ä?{0êº[o9?€Õ:ºÆá?{0êº[o83FGL J1220.1-3715@rAc@93MjOÀ:š¿3‡À;½ò×"'%¿ÎDn?´Üý@
ää~`y@_ßÿY'í?Þu`ZÄØÉ¿á· "IÖä¿â€BÌ=¿Í]ßØ\UNASNonenone?ïö.žwv?VƒÅ¸¸?Sé¢Ã…?VƒÅ¸¸?ïқÞ>s?€6"—xåº?v²à÷F–?€6"—xå»?ï[TuÏ&É?ŒƒÓþ,QÖ?"•qF&á?ŒƒÓþ,QÖ?ïÜP®;?h䝸*ÔÞ?q×ý¨â|ÿ?h䝸*ÔÛ3FGL J1220.3+6055@`4'¾‹Áj@Kå~ºñ6À:ņè¼í\À<  ‡Êd=?¼"Ze@9»n€'@#?¥‡d¿åùáéû˜¿éÙ¼06Bv¿ìv'"×?âK˜N­kUNASNonenone?ïÑùÇÎ1?ŠÇí~®Ì?w{ƒçÑ?ŠÇí~®Ì?ï¡Ø"ã¯?—¯n'"?‡¾É÷G7?—¯n'"?íÜ[ÂÜ­?¨¹Ã{?±!é"{?¨¹Ã{?ïílÊÝá?iBø·6¼¢?bâ"5"2?iBø·6¼¥3FGL J1221.5-0632@ri$ò'Ð@KÆ YžØÀ9b+åaIÀ;'ÍDÁÐð?æöËA˜Œå@±VPÇ!@ÿ"_mλ¿Ý-V·$x¿ßìj…ôù¿áû`Þè]¿îÍ¡¸ÄN›UNASNonenone?Ò'jl+?Ǟæ¤n¬?æþ|·JÉê?Ǟæ¤n¬?á-"!êD?ÐvQIȬ?ݤ÷¼+ß{?ÐvQIȬ?ݞV)~e?½%;,ù<¦?á0Ôë@¸N?½%;,ù<¦?àø~¨U¸r?¸»H€«L¢?Þ¯T?¸»H€«L¢3FGL J1222.7+7952@_ Ò
ú/@B–-û¹À:Â3|.NÈÀ<%K#É¿è}ê!Ø~@ÅXlþ†?ûËÓÀ±ád?ïî·JÚnÌ¿Ü&¢¡U$Ë¿ßrøËXX‡¿¼ÖçzDŒUNASNonenone?ïù•<ï: ?RÅÃçƒ?I«C2?RÅÃç‰?ïÑABxñ?ÀR˜†E6?w_^Ãô‡½?ÀR˜†E5?ï<]œÞV"?'"ä«ey?˜tLd5-¦?'"ä«e{?ïþ0¶Ô¶?+…:
.?,ôžB´•?+…:
.-3FGL J1223.0-5622@r¯®]á\§@Š\å´$À9_7T*#ÀÀ;AiÂ;yS?è~Õp_c"@"üÄâ@4Ô@®¥¿ç£Äë¬â¿ç7Ì@\¿ìð³'ÎêοçG¾É1•WUNASNonenone	?êýêP'ðJ?¿á`*ý³O?ÄV½¸>Ú?¿á`*ý³O?è|Y»ì?ÒèÞºù$…?Ïö™O?ÒèÞºù$†?êKÌ^Þ?°1љY?ÆÐ΄‡·Ã?°1љY	?Ô˜îóDÅ?¼,éq{eø?åñ³ˆ†]Ÿ?¼,éq{eø3FGL J1223.2+1215@qY ¥&•–@Rn•¿ðExÀ:Uÿ'E7BÀ;Ôzª3?âæêÖUÀ/@
^)Òâ:@´ƒàtÊW¿ë¸Kwn¿šº"|È¿ãÆÔ²–¸¿êjx"nëUNASNonenone?í^8'uØi?³¹dãЖ?µ;ìQ<´?³¹dãЖ?ë–&¢!°Ñ?؏…¥?Á§ewy<¾?؏…¥?ꫯœ<d?²o«ÓÀ@À?ÅQBq?²o«ÓÀ@Á?á×®b§üj?¿K»{ë —?ÜP£:°*?¿K»{ë —3FGL J1223.3+0818@q¢éxÔýô@Q'êžnëpÀ::H=†sLÀ;ËÿwD?áP½R¡Û@
÷Ú·R?ÿÁìžú+«¿å6l³)(¿Ä¨M ‹•¿Îy¨çH¿ë÷4£[ö\UNASNonenone?ê3bÔêóþ?È'/{߂Õ?Ç2t¬T0?È'/{߂Õ?ë½'aO¨?Ć°"œÎ?Á‰¶zÁ`?Ć°"œÎ?é6=Ó¿þ?¸Ò{ ¬'~?Ë'§±?¸Ò{ ¬'~?éÿÍ4]?¸t}Ãۇ?ÈËë.‹‰?¸t}Ãۇ3FGL J1225.4-3448@rŽg ù	l@;†ƒ<`À:ºèÊYUÀ;á'o°'¿ô±ó:ß¿@1PÊÈ»›?ü'ºž÷Ò_¿Ö25ÿ¶¯¿É3Yö¸Ðä¿ß­[ÿkl?»}ÙI²ÑyUNASNonenone?ïòa¹ˆ!Ë?b$œ<õh?[<Œï¼iH?b$œ<õf?ïÛH"Ý?}\nF€W?rtÛ¿n'«?}\nF€V?ï1¯
ûJ'?õ1Í=S?™Ê@–­ì?õ1Í=R?ïÿ?1Åi?ɂÄR±?ÇRސø?ɂÄR°ù3FGL J1228.4-0317@r;jžnëp@M‰‹ÖbwÄÀ:ìÝäLEÀ;¯
õ´MÀ£$u«'á@‹ÝËø'@,û GH>¿Ìˆ©'
.,¿á™âGeù¿ßX#¦ô¿åôŽï`d^UNASNonenone?ïÔ
sypq?ƒÂHö7/?uúÆCGÇi?ƒÂHö7/?ï×\=´?†Ø¦63?t}QÀa&,?†Ø¦64?î,¯À(‡?¢î÷qm®|?­>5ýw'?¢î÷qm®}?ïÿÿþOËJ>R
ËX8S>+KvuŠ>R
ËX2™3FGL J1231.6+4825@`{ԕ*™@Q`þG™À:Ø£š¤À;»‡Ý¯s ¿º'÷‡
¡@WÀ<pž¤@À‰G'¿å&ËEä¿åV c€`–¿ëQšfÜó¿ÛGÎûü[UNASNonenone?ïóŒÀæ½ ?cW#µ)Do?Xæ~2"Á?cW#µ)Dn?ïzÚχ¦D?ŸjóцË?¤¦7?ŸjóцÌ?îåÉ"ôÇø?˜R+
el'?¡£mг€ƒ?˜R+
el%?ï6)ØV?"4x¹
?>ÄõD?"4x¹
3FGL J1231.7-6513@rÍ×süPÀqOøÃÌÀ8Ác¡ À:ôóW{?óñKle@üóʒŠÝ@e#?ö;¿àÐ9zŽÖ6¿å¥+XÚs¿èd1®ßã¿î‹ºù¥)UNASNonenone?ƒ%Qþu|¿?Š%õpê?ï³j¸*
?Š%õpê?‰rýŒ˜ºœ?¤¿d'?ïš4	͝?¤¿d'?ƍªR³@?²Îi'Ø?ê\•kS/ú?²Îi'×?·1 G®^?ž'‹Ôû)¹?íÛ÷
4,?ž'‹Ôû)¹3FGL J1232.3+1701@qeŒûüeA@S¾7`¿]yÀ:K1"·ºíÀ;·­AJÅ?µR"Ž49,@
» ì^¸r?ýeÀÂ}i?â÷ñó;»1¿Â½¾ßE¤¿Þ}4B@±¿Û¹'¿ÚÃRUNASNonenone?ïÕÌ°9 [?z*[´Ý-?u§ã/Ò`?z*[´Ý-?ï"qÛy'¨?—Ÿuº?Šã‰!¶?—Ÿuº?ïj®Ã'f?'æ>VB?œòª'Ó-?'æ>VB?ï
Kéû´Ù?"Æ …ˆ?žV'À‰dö?"Æ …‰3FGL J1232.5-3720@r¬r䎊r@9`œä§´åÀ:Eä9ÐÜÀ;Ã3{W3¿ËÝ«Pj‹@#
%­c¦?þ˝_¡Ñ!¿ì¾WýJ¡—¿ÍpºZâØ0¿Ù2҇™3e¿Ô"•ziíHUNASNonenone?ïýw!U?;"ÿl§ßá?4GÏÖõY´?;"ÿl§ßð?ïÖ,‹<h?#Qd`#?téºpaÌc?#Qd`%?ᅱ¾†sZ?}BÊhóÂ?€P^c){?}BÊhóÄ?ïò00'eÕ?U†tÃ;`?[ŸžÝ4V¨?U†tÃ;c3FGL J1232.8+1332@qÅ)ûçl‹@RîÐ=š•BÀ9þ©1½nÀ;'ÆÞOâ?֕YscÏÞ@o÷oF@]o€–hb¿ç{YŶy¿äœo
éÓ¿é{€cŠ
}¿ïþ2£nQUNASNonenone?ï½4lå3Z?'þ¥N­»?€²äƳ)_?'þ¥N­»?îÜY¨ž?µØþøm{J?®¢:e~–?µØþøm{J?í¤%kÑJT?¢Äè.>W"?²ÞÔ¡u­c?¢Äè.>W"?撢‡§ìŽ?»·%ρŸ?ÒÚºð°&á?»·%ρŸ3FGL J1234.7-0437@rqe"¯O@LÿŠC»@³À:ŠE{4SÅÀ;³"¢Ù´?Ùôÿ­@êI5Ó÷c?úb¿?›vi¿ïÕ@–?"b?åÝÝ*_qw¿ìõêÚBÅç?è\k˜ÕN|UNASNonenone?ï¿yˆ	iN?…iÀå'·?€!ý¥¬—?…iÀå'¶?ï¼*ևÙ?Žq	‰Nx?€õJ^<Éô?Žq	‰Ny?îÀÒ5ü'?¥,=ûfh&?¯"òÜ 7Ý?¥,=ûfh'?ïÝw'us?yiÖ¸m>?qD7~ÅF?yiÖ¸m<3FGL J1236.5-6154@rÒЛùÆ*?íSó.ZÀ93»ËóˆùÀ:Ÿlç‰çu?ȐÝ,Y›@Ø+Ú#w@ð¸`Y1¿è­ˆÖËÆ¿ã-\òÓô¿é½)Æo\ü¿áI踪oÄUNASNonenone?éøÓçO>Å?ŅʿÛÃá?È°bÃé?ŅʿÛÃá?é`ŒŽì?Ðsa¢CE?Ê}ÍÄO·›?Ðsa¢CE?æøìs-?¹€o¤Ï̧?Ò'ÝǦ?¹€o¤Ï̧?ïWP´bœ?•­Æ!³]¼?žués¬¤?•­Æ!³]¼3FGL J1236.6-7050@rÛMžƒä&À *™0¾À9Ôÿ¢³õÀ;dÎ#"¿îÎ2c»¢i@ß	»?²@©c `Ș?íM³ØØ¿ä##À›Þe¿ærQ2;€N¿ÝÒ"…¶¹UNASNonenone?ïíA£Zõ?h';™0Z?bô¾\¥?h';™0Y?ïU›ÆQ?¥•Èp|‰?•L‡5ßÏÏ?¥•Èp|Š?îKh<¾?rÜ­Þ°?«I~œ4?rÜ­Þ¯?ïüé^??ñòÜw??`µW>m??ñòܓ3FGL J1239.1-1158@r£6âë@IdÿñÀ9­Öû#ø-À;"ÙHÜ?ñ10N§X@D£JÈP;@ˆ ÀaŠ¿êä¿hìt¿ëäQZ)…ú¿ÞÇ\O≿å'UZPUNASNonenone?ïÓb²çÜ[?e>.òo?vN¦ŒÒu?e>.òp?í†eÚv¼?½˜ª¬M	i?³Ìס,J?½˜ª¬M	j?ëÕvü¦-^?«ªt®õµ^?Àª$
gJ‡?«ªt®õµ^?â=]¶YX#?Äštyy?ۅD"MO¹?Äštyy3FGL J1240.3-7149@ràÝDUGÀ!ò7Š°ÈŠÀ9NÅÚjDAÀ;PPKqîZ¿ô4ÏÅЄ<@ÿ÷1Ð1±?ÿo¤?åÉ¿ç3àÃ¥v¿ãü!‡ Y
¿ÛyVÿ§PοÒíƒ~Ø«±UNASNonenone?ïÿR~©?" nÞ?}õ°*æ÷?" nÞ,?ï]9êÆ(? šyýÄùÿ?X§:ô? šyýÄùÿ?ïҊj"Z?z3Í,?vºÀJµÒç?z3Í,?ïÿÂñÚB?®K×>þóß'½?®KÖZ3FGL J1244.2-6227@rá˜ÜÛ7Ê?ÚbÅGtÀ8¹+0/sÀ:~"Ž½ž?ñZ:MƒÁ@
°(ù°@—kˆ±j?ïþßZ)Rp¿ã6âƒ~‹\¿ædæo=Ù¿ì¬wJlé@UNASNonenone?{Ž+é½2?"ãܸØ?ïÈã¨-Ԇ?"ãܸØ?žÌD`Wێ?±ÚñÇ=r?ï	ÜýA$?±ÚñÇ=r?´$1Nù
?£øÙ¨-z?í{yÖ Üž?£øÙ¨-z?ÇýñJ
q?µŸÓ"e†½?ꃭ}c¼?µŸÓ"e†½3FGL J1244.3-5515@rޗö+jè@gB™ØƒºÀ9_ýŠÚ¹õÀ;O¦¢–˜]¿µ\)^ŽÄ@«wÈ8"o@õò`L–¿âX´^ìÊn¿çt|')ð¿êŠ'=:%É¿âE&M¼ŸUNASNonenone?ï‰fÛsø?'h¯¥h?¦I#9Aû?'h¯¥g?ï)Ì¡|¯}?¯t¦@cÛï?šÆkÐjj?¯t¦@cÛï?í̈ߍ¶±?¢Æcâ¾îî?±›¹'Js?¢Æcâ¾îí?îÈ±8!?–r)\Ü
?£>¤ì}ì?–r)\Ü
3FGL J1249.1-2808@rå2a|Ú@A\ÚãæÄÆÀ9Ý68¡1>À;ªíñ	Â÷¿ç•ÿø€§@E
6ÊA'@ˆ‹`pÙ¿èÛÃoMb+¿ß)ŸÑ`I¿Ýj…ÿLÀ'¿ÞŽk›¸
UNASNonenone?ïü÷ƒè%ã?3½¡_E@?8Cà¾Ðì€?3½¡_Ez?ïÏY.T˜?eGÊÆ	?xShôÕ´??eGÊÆ?ï̕‹Z&¾?x£D[m)Y?yµ:R젚?x£D[m)[?ï÷I=²Š?M™R2Þb?Qm"šëÞã?M™R2Þb3FGL J1249.5-0546@ràë…¸R@L‹fÉûÀ9óÔCédÀ;mQ¿tè¿àAg©\…<@³g€Â³@M¤`r¬?ïEcòmÆ,¿íc\›·¿ÀÁÁ‰¿è¥åÊʔ
UNASNonenone?ïÿ|ԃ?z3‰ÔBÂ? ùÊß:X?z3‰ÔB ?ïÀï­û/¦?Š'¬ý	 8?ˆ)h-^?Š'¬ý	 7?ïP0™ú?'gÉäô?œõùìßàÇ?'gÉäõ?ïø(|·fh?Q¶4ÿý+=?O^
"f_?Q¶4ÿý+A3FGL J1250.2-0233@rå'¡ Ï@N'=¯÷¥À:—öÅĚÏÀ;‰Øê2¿Ô!‹ôs
@
5I¯?ñ€y¿ïôÍÁᮩ¿á Í‰¤ó¯?ç³p;Á?êX•íUNASNonenone?ïþÕ)Œtã?&q)KV3?"­g8±Õª?&q)KV?ï̔ßN?‡…´¬2,?yµ¿Xð?‡…´¬2.?î¤$M:;? ˜¹gnê?¥½»,\F3? ˜¹gnê?ïÿâ©,ÝR?œ»'ù>íVÓ"­Ð§?œ»'3FGL J1251.0-4943@rîƒùd@*GЍK­}À9ÖBƒ2OÀ;tˆhî?á;­2Ü(é@¹ÈQ½âÏ@=ÍØã\?æ7€y%õw¿Õó(¼6Òz¿ÒÖ"¿{30¿é¡¿+é+ÂUNASNonenone?ìk³ÛT?»7—ÐÑjÜ?¼§ra'õ\?»7—ÐÑjÜ?ê
^Ÿ
»Ó?ÇWy섓~?ÇʅƒÉ³?ÇWy섓?꧚|	ƒþ?²'ì5°?Åa–Ùð?²'ì5°?è졻Ιc?´1œ…ºž?ÌMyŚu?´1œ…ºž3FGL J1256.1-5703@rùHè§ç@Bæê…DxÀ97¯h¸À;Ð߁w?òùéá½)@weêÀ}´@Š<€c舿æ"ŒéC)¿è-¶G¶^2¿ëûGC,òÊ¿ì/%\…èUNASNonenone?λ"+Œ?Å7DVá—Q?èQ9:u?Å7DVá—Q?âÚü¦$²?Õ·Ø&wê?ÚJ³Ë¶ž?Õ·Ø&wé?Ü´åQԃ?»ƃÊmâ?ᥱ
W¾?»ƃÊmâ?ÂKeà…!?§‹ë$ÀÄ?ëm&‡Þ¸¸?§‹ë$ÀÄ3FGL J1257.0-6338@røт©"¿è¨À~	ñÀ85«³w'À:‡/	ØÆÖ¿¤8Î@ˆr@ÿqŒ_Ig@ò]Àz"¿ìÞ—ÈšI¿ÂBfÊíØ¿âGŗé¿éY˜ÖëUNASNonenone?ïŽvƗäu?"&½—bì«?ŒbNZã?"&½—bì«?êËßf´?Ð"~‰÷é?ÄЂe½/±?Ð"~‰÷ê?ëÆåÉu"?ª	ÀÖµ[š?ÀçôhÚ)¬?ª	ÀÖµ[›?ïéú‰<3e?f)DÅ£ ?fvÃ̚¦?f)DÅ£œ3FGL J1258.4+2123@sî˒:*@Ur\=îxÀ:1—¿¤ÆÀ;'UÙPhÎ?ñ[Õcõ@%ÅäêÑ@&K_yã¿ë¾Î×û¿ïÿÕÝÚ?ïýåu²¿ä§B"èe7UNASNonenone?ï÷/>['?Z–n,%ß?Q¡áƒHÝÞ?Z–n,%ß?ï}‰†¦2\?®TeõÒ¦?NÏ+9´e?®TeõÒ¦?ìÔr×Bk'?¦­Þ›qþK?¹\iEì¦Æ?¦­Þ›qþK?î÷+"?»Rt¤—? Ž½Oº?»Rt¤–3FGL J1259.3-8151@ró¦">jÀ2þRv‰ÊÀ9Ê=|bQ.À;€ü‡7?âã"˜A'@Aà;i@'æÚ¿æäNò_1¿ã-=À!e"¿åSÐÄþø¿ìÁsnUNASNonenone?Ý~UY5¶?й"½c‰?á@ýÕSe%?й"½c‰?èð®Ö9}?Êðëðš·?Ì=G"§?Êðëðš·?遏{X}?³|LúˆÓ0?ÉùŸÞ?³|LúˆÓ0?ä±(Ù¬c
?±ȋÖI}?֝®L§9í?±ȋÖI}3FGL J1259.5-3231@s™" ä@>Rb˧2ßÀ9Œ‰B37À;p—"6À
eS®þ° @{X³|@¶™ßåƒR¿éÎ]àÓ6k¿çO¶UU᣿çZaµ?¿ïÿ	̀žBUNASNonenone?ï÷ Àž˜?VrŒ¾ô]­?Q¾~ÃÜÐ1?VrŒ¾ô]¢?ïÙm)¬Æ'?~o¡"mð?sIk)œìd?~o¡"mñ?îçÚÊ?ß?˜5ã¢.®Ò?¡'S_œþ?˜5ã¢.®Ó?ïÿè±wÍ>ÿm²<=>çNˆè3œZ>ÿm²<ß3FGL J1301.5+3333@Z1ûµsë@TÍ+©ÑöÀ9þêUrùÀ;Ö5À¬-?ïôÐp‡õ@'áÂ@-g߸6é¿ØT˜Ñl‰¿áLçee›¡¿è³vH q"¿ïÿÄoAgUNASNonenone?çüséÿä?Ìm"'cïè?ÐÐ,8?Ìm"'cïè?çG&p0M®?ÎÑC³–!?Ñq³Ÿd¥?ÎÑC³–!?æ8W吓l?·šÆØp?ӏP4ÞÙ)?·šÆØp?ÕÕè»°F?½6ŒÇnÍ?åv•¢'Ý?½6ŒÇnÍ3FGL J1304.6+1200@s³ …±…@R£öÓ0"À:¬Š7&À;¾òâ
K³?ê$.Eì&@µ[©Éèl@ü[€YV³¿Ö¹®(8Ñ¿â*5è3¿î;²[ü@¿ìÂ[¹ì1UNASNonenone?ä8‰å/"?ˊk™ `ä?׎ì5É ù?ˊk™ `ä?êèø…µò5?ɸ[v·=?Ä\é(7)?ɸ[v·=?çFЌ @?µMûãÈ'ú?Ñr^ç¿~ß?µMûãÈ'ù?×±J‡ü´?À:KbìbX?ä'Z¼ô¦?À:KbìbY3FGL J1306.8-4031@s!° ě¦@6>]ž@ÈGÀ8ñjwmçÀ;ëÃ2X¿ò]kÑ@;®õKq@SL`UÖ ¿æ¤2
$'R¿åðÎ5úÛ¿æ2ÓD
Eÿ¿íHˆ,[UNASNonenone?ì´ÚóÁ÷¸?·©Íÿ
ë{?ºY(aðB9?·©Íÿ
ë{?íº¸Vô>R?»Qµ´c.¿?²*=H^
y?»Qµ´c.À?édkÊ"?±	
cSäP?ÊoŽQ¼Õ°?±	
cSäP?ïvvƀðé?"{¡P'Q?'1'/áâá?"{¡P'Q3FGL J1308.7-5738@s4Á¨¬\@jOvÀ9`Ö@†À;"ŠfðÀ^õѨԠ@+[Àðöx@mª_åmØ¿é¡XØçÀÍ¿êöbªÅ¿ãN`5IãÏ¿å'ärʑ£UNASNonenone	?ïÁgû¯c©?ŠË@	Ðþ?L(N+Ó?ŠË@	Ðþ?ï ¥Dþ?­OpÕDþ®?‡Ö®À\½ã?­OpÕDþ®?í38ȓp?¬DÑùpí?¶f9»g܀?¬DÑùpí?ïüt–70?M¸Ò³úG×??<[NF~Ý?M¸Ò³úGÖ3FGL J1309.0+0347@sžoü]ö@P'`A‰7LÀ:—10#´:À;ð3PD¼?ðÄð_y@íyj¥@¯i\e¿ãS÷‡û%j¿¹U&œ"À1¿ÑÒÛ
8yT¿ïû|Ë`DUNASNonenone?âb×Á	¶?ӂRP²k?Û;úP}ì'?ӂRP²k?ãaÚ׫ó?Ôgƒ—GÉ?Ù<KþP¨?Ôgƒ—GÉ?áTÌÔçw©?¿=‡c³Äù?ÝVfV1®?¿=‡c³Äù?á| ó¶…h?ÃÕê(o?ݾ'õ/?ÃÕê(o3FGL J1311.8-6230@sœàuöý?ÑW«ãs,rÀ83¸"0¤À:,[Ðá."¿Ð GÑ®g@©h­¾i³@ªÚÀ«VZ¿ãH4qC0¤¿èðݯte¿ä=`
¬¬¿çõȝNk.UNASNonenone?ÖFKA\ªw?ЭŽËTP?äÜÚ_QªÅ?ЭŽËTP?âGîÄ8ç?Öìý˜Sh?ÛqÂ"wŽ3?Öìý˜Sh?ááã}GH?·'xÍ­ðx?Ü<9÷qr?·'xÍ­ðx?íŒR²ê?³~¯¶?³o"h¯s?³~¯¶3FGL J1312.3+8513@^šâ:¸c@?á鞔«À:5-ø`ÏNÀ;ޓ*êU?Ó-}*'èº@
ì¯úÙû_@Œrk­¿èRÔÚs«¿æPÒLàѿ旤ØÿпÑÚÍì\ŠUNASNonenone?ïòŸLÉÿ,?du©ÈóÌM?ZÁfl§ø?du©ÈóÌM?îBM%»æZ?¶;Î↙?«Û-¤Aš\?¶;Î↙?$Ö<ù?›2Pá'?¦4²œ0s?›2Pá'?é	°7óÈ?¿5Ý
Ðá?ËÙ?#€0ã?¿5Ý
Ðá3FGL J1315.7-0732@s—+Iº@Ki¡lçŠÀ9f'áÇ/ÕÀ;'N+Üýœ¿ú0qÅ?9Ò@"étù&@'JßÍ/ž¿Ìß³={¿ß,Lâx8¿åœVK·u¿Æ·ŽgUNASNonenone?ïîBIL1?eÚÂ˱c‡?a½¶³óÏ?eÚÂ˱c†?ïʏ&õj×?ˆîÞÁ7i?z¸l…J"?ˆîÞÁ7i?îÅ7»›¸?™ÂôÖ.;ú?£¬"FD'?™ÂôÖ.;û?ïÿÍ%ÊD!?A­gd¨'>ùmÝï2N?A­gd¨–3FGL J1316.2-6446@s/D')‰À3¼$ÞܚÀ8{¾öJt˜À:Åe˜Tö?à;'1ÈúÛ@¨/t··è@O"/û›¿èeà
éš¿èd€k'ôÄ¿ìÈ`´u½ò¿áÝüó¹©7UNASNonenone?豈VFÈî?ŒÊhÝ9?†ßênMĬ?ŒÊhÝ8?í£'òvé?ºáÔêO˜)?²æÇlH­?ºáÔêO˜)?쉬úi†?®jWøÊâ‡?»²˜,³ÏØ?®jWøÊâˆ?ï0:=ãúî?ŒF†Èßp?™ø¸C€¢7?ŒF†Èßo3FGL J1323.2-3901@sZ‡ÝDU@7nhãï(AÀ9ËøÁG^À;q½OH¿ÙõÜûîùG@ŒÖ脎@.Yßð@¿ãÍZÐc–¿èœ±ûÔææ¿ã`C˜õɊ¿éh=2v±UNASNonenone?ïèY¹¢ì?po@•.,4?gç¦F])?po@•.,5?ï…hß3?¤£Éš©¹?RäùŽ?¤£Éš©¹?îƼÂõÙÑ?—Y£1,Z…?£"3Тbï?—Y£1,Zƒ?î"iÔú%?CÚ'—µ?¦¹b°]®8?CÚ'—µ3FGL J1325.2-5411@s>¼¾aÏÿ@ ·;dZ¬À9AŒa¢²GÀ; èN2'ú?íñ—Ú;w@¥®¯*z}@Ì€•'¢¿Óÿúܪb¿ä=,°sa¿éX ÌSU¿ïÿÙ14*UNASNonenone?Ӂs«˜ð?Ìeq) U?æ?xF*3ˆ?Ìeq) U?²Ü"žëZu?Ä9,C6Û,?í¤{¬""±?Ä9,C6Û,?Ù%©ÃÈ?·:§	«³6?ãm+u}œ?·:§	«³6?®%ª]C~}?—ÂýWçö4?î¥Z+È?—ÂýWçö33FGL J1326.2-4651@sQÀ­Ú@/4ƒì‰*·À9ÕÜ@WÀ;0¥:·‹ó¿øÇ6þCè7@
²¨óSÊ-@Ž— <A?ïíȬýj¿ê¿«aB:7¿ïþÍë'MC?ïó
ƒ½²UNASNonenone?ïüÓöȒ¬?H5¾ÿè?9`I»j¢è?H5¾ÿè?ïãml¨\Û?wû^)͐?l'"W£%8?wû^)͏?ì±À<P]?¨bÖÏgA?ºqÿv}?¨bÖÏgA?ïÿ䢪I>þ5^F^_>ë]U¶î<q>þ5^F^¤3FGL J1329.1-0536@sþà"'@LÆ)ñkÀ9ƹ#¢œxÀ;@2芘u¿Õ?Aì@esˆ¸Ë¹@Ð
€CR¿à'Z$—¿ã°q7!C¿ààAƒOw¯¿çt¯œ\¹âUNASNonenone?ïúy"SâJ?K-¹†Q
?F®°vÜÑ?K-¹†Pÿ?ï¦]Ys?j	~×;¼?†hº)£8'?j	~×;¼?îÎ],ñ§?—èz³˜ZX?£-0çåŽ?—èz³˜ZX?ïÆÖ³sÙÉ?uYKEËP?|"¦Fˆ?uYKEËQ3FGL J1330.4+5641@\
gbé@MТ ©XSÀ:dš,fXÀ;øwéE©¿¨Q&#°RQ@OƒNÿl‡@öê?yg ¿å,öŽÖâ¿î–56¿¿±^:íU/¿ä!q)búÌUNASNonenone?ïÿ(
Ô/ã?b­àd#?þEz"ú?b­àd#?ï®PÅ%«`?Eaࡤ?"kζ•'ü?Eaࡤ?ﰊ|ߒÁ?'þ¡–MXÛ?ƒÝ`ÈOÑ?'þ¡–MXÙ?ïì±ì°(¶?bi}-Ûa ?cNO×IS?bi}-Ûa 3FGL J1333.8-4417@sn#9Àëî@1í…zþ£ßÀ9žs;`ÿÀ;R`ÊE3¿úœ¤cL*¦@ðwÆO@}þÿú̏¿èj!Ù­l¿ìFÂer ¿Â¹­åoÊ­¿ëÝg:UNASNonenone?ï÷Šù÷Ù?]Úê¡Û/?PêMúÏ?]Úê¡Û5?ïÞ")_Ÿ"?z»ù°|­?pîëP0oE?z»ù°|­?îB%K`é?š'æÊ5$a?§+Ý«Iñc?š'æÊ5$a?ïþ¢æ?2<ë[§M?%џ6þ½o?2<ë[§M3FGL J1334.3-4152@svçl‹C–@4K=áâއÀ:–ßY—KÀ;ºXVk¿ªmyÝ@
4yeqžÔ@

ŸzÚ¿ÃB¿­ªr°¿ïþ¯€ê(Ü?ïè÷·uçR¿ãîüúD³UNASNonenone?ïû:Q¥i6?Jæ™ób""?C¹j[%7?Jæ™ób"*?ïÙÒCjcd?}Àb[g·@?sÞJÎM×?}Àb[g·A?ïpK`¿3?‰! `'¨?'öŸ3è´?‰! `'§?ï÷9Æ,cü?t´[	?QŒs§8	¡?t´[	3FGL J1335.1-5655@sNSŽóMj@Ã֞ݦ9À9ŠÙã5ÅÀ:þIc `É?á¿0rþ>@Å0Pª½X@´8àœ7"¿ßî·§»_+¿åÚä_ð¿ÝQùX,M¿íö‹ÅùýeUNASNonenone?îFÄ)"²T?­P%ûÜ?«"½g´Ú³?­P%ûÜ?îÓUt9*‰?¯{rR%]Ð?¢Ê¨¼mWj?¯{rR%]Ð?è¯.eû?²R§')?ÍC‡G'h?²R§')?ílm6¡"Å?¥nÏ	ƒÇ?´œ–JóÙÕ?¥nÏ	ƒÈ3FGL J1335.2-4056@s|quŽ@5.©÷µ®£À9R%cf×¥À;Ov©ªˆÕ?ÉAy"÷@]EÀÔq@p[­Š<¿çÙ|Oa¿é㼊àCL¿å艧ÝÞ¿ÛnÝzUNASNonenone?ïß%níqˆ?rSŸCwaW?pmH‰G;ç?rSŸCwaW?ï‡øâa
N?™iîüé«ý?ŽÇg¼¬'?™iîüé«ý?}ƒÇê?ü–"
m-?§8'ÁZ?ü–"
m,?Ιqµ?—£ò3P«?¦hä²?—£ò3P«3FGL J1342.4-6904@s7ÃAž0À›s¢¡À9§vÖöò:À; ãœòên¿ìÃ4ø@È-*Ûv@8¬Ë¿æöfÏþõ¿êô³|>¿ÚËàiÈ×±¿çج˜5&ºUNASNonenone?ïû-VXA¨?P÷	à×Ìy?CJ¦žù_¡?P÷	à×Ìt?î¿ Ûۂí?´ßt+Ð?¤òBGÑ8?´ßt+Ð?îìÆðÄ^"?—l}¥'Š?¡3óºÃ?—l}¥'‹?ïâX|ò·?mÀ ÕfuÑ?m§ƒ
Hâ;?mÀ ÕfuÑ3FGL J1345.1+1949@}Èû†ô{@RìÉ.À:?|èˆêöÀ;Ïòü~¹¿Ø†
á/…@mìðƒ¶@Ò.@Z80¿é…U;¿æa3æÙµ¶¿à¨'v'È¿åìb?vs¶UNASNonenone?ïÿœÊrȨ?"Ö1j›¼?ÍcMÕà¢?"Ö1j›¹?ï"ñ/(SA?›8c‹ó²)?‹´5ë/â?›8c‹ó²)?ï°ü,:Ùî?'7Og#ü?ƒÀôñI"'?'7Og#þ?ï³5wóï€?{Ø}4Ï?ƒ2¢ô?{Ø}4Î3FGL J1346.2-2608@sà)~+V@A'Ó"vóÀ9êwXüñXÀ;³$™<|ˆ?è6'Ú!@‹£š#';@›'`—¿ä•ë8âí¿âÖ^¯§è¿ãR]ƒG¿ìÂ,G(*
UNASNonenone?ރ¢§³òÈ?Ì£À'Ãt&?à¾.¬&œ?Ì£À'Ãt'?åéwŒÜ˜?Ê©~à;ä?Ô-ææFÑ?Ê©~à;ä?èÞ'Ð.?¶ðÑëMt?ϐ"õ´¿I?¶ðÑëMt?Ü̗ٝíy?»cuòøQì?á"1´	D?»cuòøQì3FGL J1348.5-7150@s6t¼j~úÀ"î%¦'¶(À9¼ÚH¶RÀ;ZÐW›È?ÚÉN[5cm@@&=+""@€¥+ô¿èWt4¿êÉiñ5aâ¿Îž.bج¿æêÜØ2±ƒUNASNonenone?ïÿ
´Ju­? ­V±J•?©v±JF? ­V±J•?î†v'àÄs?¶sßÒ¸cÑ?§˜ó¸×?¶sßÒ¸cÒ?ïŒÑ˜
Ö
?Š´Næz"?ŒË™üŠ}ƒ?Š´Næz"?ïª3ˆP‹y?€òED{U?…sëÝ!«?€òED{U3FGL J1348.5-5833@sezÁҝÇ@ß°&£Ø¸À8ô´JÀ:æ$óÅ?´¾ÛÚ.@âøc!@XKŸ©†¿êL:­>ÖÄ¿êYãñ#ǿ׆£˜ÞÖ¿ê¤{X™}UNASNonenone	?ï[Íóú]?ž×ãŽ,Ü?"†A€¾4\?ž×ãŽ,Ü?î€Sí*-\?ºFÇúƒ{?§úÁ-]*E?ºFÇúƒ{?ëOU/ƒ?­éÛÃÂ¥?Âú«ƒAô?­éÛÃÂ¥?î_ºø¿b?¡¹£tó?ª4Pt	Ó?¡¹£tó3FGL J1351.1-2743@sì^_0çÿ@@§T!ÀD(À:¿¦¥òÀ;šCV–势öÀ)æ®JV@!¯B"dY@c cbP¿ÞI]褪ֿì?ž8dË\¿äóC¶……¿¹~"d%EUNASNonenone?ïýƒxST?>ÝI¶bÊ?7Cä=e\š?>ÝI¶bè?ïÙ¬N$#?C?֗ H?s)ØíîT?C?֗ H?ïbŚk¯?—tW&e>?Ÿ"§L²Š?—tW&e=?ïÿ"ÿpÀ?; e4§j?À#Ïý?; e4¦ý3FGL J1351.8-1524@t;Ýcˆe•@FZ³R¨À:E{°z†¯À;•
ùXF¿ËùÈä
4@Ğ×F"y@4`JmŒ¿ì¬ €Ò[¿ãçäeI¿â`ÇúfIF¿ÕùÅÈexÄUNASNonenone?ïÿÚUu?"ù¾‰Ñ²?µNQn?"ù¾‰ÑÑ?ð"¿?™S/a÷%?ŠCÞÐ;?™S/a÷%?ïƒ4×½ü?‹Oí­Æ?2Ê€úÏ?‹Oí­Ä?ï媯3?e:Ǿcß?jUPùéÍh?e:Ǿcã3FGL J1400.2-2413@t&©Ür\>@BÖ¡aä÷À9ÞvlmçdÀ;¤ñ-À?ó¨›C@U;ÉÇ_@@Óàx"¿åÞ÷*T£'¿Ñ²Å1u¿äÈò¯3<¿ïÿúÐÚè2UNASNonenone?ÓÉaì?ÓWÌ#ùÔ?æqÿO{Š?ÓWÌ#ùÔ?Â,D¡§¢÷?š:½eBÊ?ëtîזB?š:½eBË?έ
)g?·áÂ>ÇÑ?è|º½u¦?·áÂ>ÇÑ?Ãd¨%D?¨…æî>@?ë&Õøö¾ð?¨…æî>@3FGL J1402.7-3240@sþ=ÈK@;ØÃÁ‹P+À:-bŒ½EÀ;´ê8v¿×wò.J@Ìdȵ@‹\@r¶×¿å*±Pg¿ç`ƒ<ØE¿é7ÞS¿âçƒ(áUNASNonenone?ïø´"6/?T"¦¡Þ?M-³'Aþî?T"¦¡Þ!?ï²vÊ}ð?Ž˜l:&ŠI?ƒx¢M`ƒß?Ž˜l:&ŠK?ï2šŽž?'æ3²Y?™¬¾Ž,?-?'æ3²Y?ï±Û±Q"?zØÅß*-=?ƒ‰?"«žø?zØÅß*-=3FGL J1403.1+1304@vH'ýuâ@Q—á2µ_À:Ájî‹À;ïQ{×?éüQ·Øžè@ÄîÕÒ°@ +ßVè¿äÏì‡cr¿Û4¸#G'Ë¿è|&x¿ïÿ"¢[VŠUNASNonenone?äƯ¼É '?Îá§I‹ñ?Ör †m¾Ý?Îá§I‹ñ?åÉTþ',Ó?ÏQ͂Ssr?ÔmVݦY?ÏQ͂Ssr?ãü"a7÷S?¼fÌì?Ø÷=Z?¼fÌì?Õßáo³¬Å?¼í)$dË?åH&)ž?¼í)$dË3FGL J1404.3-5241@sŸ¬1&é@!4úïõÆÁÀ9²ä¥5¯À;I¼2JÕç?ê­-°Åã­@ޒr@Щ¾€¿é½«û#«¿ÔÍ6ŸNdg¿ì/¤`p¿åL²Æˆ²UNASNonenone?ë0û$»'?¿£Üã'Yž?Ã<oÝe?¿£Üã'YŸ?í5{\GK!?ÄlS	9?¶T%Ŧö?ÄlS	9?걔X;m?°!v;@ù?Å9¯ÂŸN?°!v;@ù?æ'ãõE°?º(šÒ%?ÒÜ8uö¡?º(šÒ%3FGL J1404.7-5844@s…d2‹n@Ki~J‰À9ªÂ©][üÀ:ÍçâÒÉ?І5lQ@
Y»~Ư|@U]ŸÃTS?ï=p?qô©¿ìñ£êƒ¿ãv˜@[ÿ¹Þ'$¸ÏUNASNonenone?£Ñæ?•™Eý¹?ŠW»Fn?•™Eý¸?ï/vVÿ?¯ìNscD7?š5<À?¯ìNscD7?ìø,TãPà?­÷8ãsTÒ?¸>Xåxú?­÷8ãsTÒ?ï'Fwµ+Ó?‰©ºKP?‹®bµ,?‰©ºKP3FGL J1408.0-2924@t%܇Tó@>'Z³R¨À9®`À48À;±£|qk?ó13ú-ƒ@pù½EÆ@|¾`xe¿äÂÛ­÷ZÑ¿ê(߀6NÏ¿ìû+–¿í»ÓáûvUNASNonenone?ۍi¤:æ?ÊS+Xê?â}9K-âŒ?ÊS+Xé?ÐS'!mt?Ð
¹L´Ö?çÖ?6ïIG?Ð
¹L´Ö?â^A $À‹?·(´ŸƒUh?ÛC|¿¶~é?·(´ŸƒUh?­7è!Ûú?-"-ð×~?î,±}âA?-"-ð×~3FGL J1409.2-3743@sø!-w1@6¢DAxpTÀ9ÂÏL
ÑÀ;•e×y¿ïݦXނ@1›Â"¸Ú@—Iÿ¨lE¿ç<Õã™9o¿ä•ìÐj^¿èPâèÂø¿ïÿ‡{£©,UNASNonenone?ïÃ×aý-
?€ùËǐS?~OizË?€ùËǐT?ï>è(Ê? iHݼ•?˜"ýzæ½e? iHݼ•?ílÖA‰ö?£IòõN!?´ŸÁMó°N?£IòõN!?ï Â>ViF?†-'Ë­ƒV?‡Ïpje®Þ?†-'Ë­ƒX3FGL J1410.9+7406@\ﰉ 'R@DòF¿2/À9›ÖøjÀ;ûœGÉÃ-?ñ(ÆGÍt@.rÆÆù@Q_Vý"¿é÷£Öâ¿âEu³"ô¿Ô?Èå.þ¿àOœ&€ŒUNASNonenone?íj\©î?¸Ò9óà?´¯m·P?¸Ò9óâ?é¶EãÞ<Ë?È®Ót`%?É&èp‡Ò?È®Ót`%?ë‡ï¼ì?«é#bJ?ÁàC¯±V?«é#bK?àH$6_œA?ÃQ—s‹"?ßo·"@Ç?ÃQ—s‹…3FGL J1411.1+3717@QFȟ@¢‡@Q—hƒöèÀ:nêžnëpÀ;ü jÓ?ÙÛ3tì!@
¾¤B¿î@ÒäŸý5ö¿évâ0Ðò¿è×Ýú#k¿åÈ-§iL0¿ÉÛ9B†UNASNonenone?ïóO'vK?d³÷—ªŽ?Ya±iýò?d³÷—ªŽ?òT?œčåIÑ?~[êÊ?œčåIÑ?îî|cYy?•Kå[Ÿ+?¡9Ç
hy?•Kå[Ÿ+?î§Ï!2^?Ÿ}">Ø­?¥ƒýìÚ?Ÿ}">ج3FGL J1411.4-0724@tñ ä¶1@I3]9—À:†ÖHv'À;³c"GÁ¿æ¶twºæ_@ñGÊDj?þ]Û O@Z?¬U#I»?ᚌF'Š;¿â¢át';¿Ñ-•ÇIwUNASNonenone?ïájx©Ë?r]ä5Ò_?n•‡ûV53?r]ä5Ò^?ï'
š¤Ív?ŸÀï—>dQ?‹|™VÌ¢¸?ŸÀï—>dP?îÔÙôóå¾?—D&¸)}?¢²`°Á¤?—D&¸){?ïçFiù?Ü?i›arã?h¹–À$-?i›arã3FGL J1417.5-4402@síÒܱF_@0&s>»ýrÀ9W€•ÓÀ;h"¡T¢?ؕ0›JÁ@&"~…@óQŸÚÑG¿ä'DˆÆ¿¿ãò[/Y=¿â{Ë¡dÐJ¿îØv°zJŽUNASNonenone?â…]Ra¶?ÊTïéŒà{?ÚõEZå<"?ÊTïéŒà{?éSþ/Õ?Ǻ¾Fµµí?Ëú°@«?Ǻ¾Fµµí?âsF§k?À«ï=¡ÄÓ?Ûr°å)Ç?À«ï=¡ÄÓ?èKz¨P'8?³Õ1d´/?ÎÒ^½÷!?³Õ1d´/3FGL J1417.7-5026@sËË)^ž@$9¹×ý'wÀ9u΁eÆÀ;7E¶Ãv¿í‡‰½AZ@
­^܄OÛ@âZߟO¿ë!ǕLÐ5¿áuV^¹ýE¿çMe—¿á÷¤DîGUNASNonenone?íÁۇ'¥1?²á+ŒIÍ9?±ñ#ÆÂÖw?²á+ŒIÍ9?ïªõ3lí'?–0v'±?…B³$ěd?–0v'±?ì¶-'x!?¥QÑ+ó?ºN–ÇÜ>ø?¥QÑ+ò?ïÎ	ç_[?w@c˜b1?xõ{PRw?w@c˜b13FGL J1419.1-5534@s²³œ¾à@Ê'ÿÀ8Úoõ—ÇÀ;õ€J=;¿éݬý4Û@ÏJ€Æ@‡·ßªÊï¿ê˜úpQªJ¿ê~­øvHÝ¿ãèw¿êÛqÒò´UNASNonenone	?ïáýºBõ¤?qÚ-?˜@«?nE½
\×?qÚ-?˜@¬?ïà-Ā!?¡;wÔöô?ˆ‡ôŽßø?¡;wÔöõ?믉ˆÖŽö?«Ã¦
ƒ(?ÁAÙÜ¥Ä'?«Ã¦
ƒ(?ïÝ@V;µR?o$÷gmìÅ?q_Ôâ%Vð?o$÷gmìÃ3FGL J1420.9-4615@sê±[W>«@+¹ò™0À9'Ùe5À;i@։äñ?Ð'ÝßÄ¡/@
Á¬œU¶–@›¥^¿ÿ¿ë"¶å@a¿æñQïê¿ä3½6¬º^¿êÌádßR¶UNASNonenone?ï	Zr§7¬?¦ù7'Nâ?žÔ±«
¦?¦ù7'Nâ?î1Ù¼Q¶?±pŒÀJ¨?¬îbd:äž?±pŒÀJ¨?íºi'Ñ?¦öö9:?·*,³é{?¦öö9:?é3"Cbå#?±kªÔö‡p?Ë1²òtkw?±kªÔö‡p3FGL J1421.0-2431@tzzcslß@A¿"ÀiÀ:…îÁêÀ;²';ýP?ìPó/›@Mk›Y:@šÂ?U*?àZ¶_ևê¿áü»yµšù¿åÀ/@Æè¿ïÿ÷,OqáUNASNonenone?èÃty‡d?ÌýänƒÑK?ϼò.âq?ÌýänƒÑK?Õ4ˆ'Š[?Ê,xSÊý…?åeô»¾ºÒ?Ê,xSÊý…?â''ˆ+Õy?ºnï~á?Úû°ï¨U?ºnï~â?Õ!n,&9?³z‰˜Ùÿ`?åoHñéìã?³z‰˜Ùÿ`3FGL J1421.8-7920@s3.œË}AÀ1;'`4PÀ:0«ÆÂǐÀ;¨Ò3>î?ð™@Ù9Í@0Ç˱ç@&@tdV?î àç?¿äªÔÚ.×{¿å½'T«ÓÙ¿ê«';…UNASNonenone?æ¯).ÝêÉ?Ì¥^½Ì?Ò¡­¢D*q?Ì¥^½Ì?蠉Œ¢?͏ͭ´@d?Í}ۃÍx?͏ͭ´@d?ß
í×1&¼?¾"¥G€?ày	gl¢?¾"¥G€?߶'n½­?ºÖÜl‡­?à$ì~H¡)?ºÖÜl‡­3FGL J1424.3-1753@tÁëíúCþ@CԍûÖ¥"À9äZ#bØÀ;¤Wë‰P¿Ún,£¢%@1s0Ï*Ë@c]a#Ü¿é\~éjl¿ß'"®iÏ¿ÞÆÁk«ÛÍ¿á§ù´"û-UNASNonenone?ïü"?«Xœ?75‡£+³|?;^¥;'»?75‡£+³¢?ï¬zÑå‡?ŒV\c1y¼?"ùaK†ž5?ŒV\c1y»?ï´o±ó/O?'ÔµV	—5?'äƒ4,W?'ÔµV	—8?ïàÛ?L/¤?eÕöd@5?o$À³Ð[Ù?eÕöd@43FGL J1427.2+1610@'.'O"}@PPe¾ ºÀ:¤.™À;ÅÏASCÀ•Öé±4@;cÃÉÃÙ@O?ƒM¨¿ê/¨+º÷¿èƒžNEn…¿æ‡iJ"Äe¿ïÿqñp+rUNASNonenone?ïý´w, ²?4RÐ#è?2\Fžúm¼?4RÐ#ç?ﳄÇ[?"ÅR;b.?ƒýÎ)>½?"ÅR;b-?ï='ò5C?ŽÖ.î\ۈ?˜MÁ¹\7 ?ŽÖ.î\ۃ?ïýؔÓ)Ã?9àþ?1;Yf±êÏ?9àþ3FGL J1430.8-4434@t'œàu÷@-•Ã½Y'CÀ9"Ü%/drÀ;nú|2€†ÀknY$	@ø¼—u}@Í?†'Í¿ß×ólàf¿çIš†\.¿ÝvÑӜʧ¿êYIä5Û?UNASNonenone?ïð¯3]ð?a‡_»Å]"?^¡˜áD ¨?a‡_»Å]"?ïáo Ï^?y¦+oÿyK?n€ß0¡ ?y¦+oÿyL?ílø!›)Ä?£¦ygŸf?´˜>ó&±á?£¦ygŸe?ïÿËÞƛ4?"¥¿áôþ>úœ²f?"¥¿áõ3FGL J1431.1-6425@s—¾ß¤@À؅Ó7ëÀ9K¼šO¡ÿÀ:þ¹™aÝ?æú¬ä•T@›5sñ@»Ÿú[Ñ¿æWþŽ]GÑ¿ê|˔WT?¿ãÀ+Ê^3¿ïÿÜ¡"œZUNASNonenone?ïâJô¶ä°?~®bQ"Ñ?mµIP?~®bQ"Ñ?çÐþ̦V‡?Ыʇy­/?Ð^f³Rò?Ыʇy­/?ì†ÔÄ'?¬Qv•¬‹?»ÏYßÉ?¬Qv•¬Œ?êIÄùFô?²r+ö\«ñ?ÆÛÌìä4?²r+ö\«ñ3FGL J1438.6-4209@t5K}At?@0lˆçš®mÀ:
xë¤(iÀ;fûéðÊ?ä	©`¥Ì@+-Ïqï@'¸`.>¿ílŸæe¿ä½4ºƒ¿ÙSÞ%²
¦¿Ò¨"^F\[UNASNonenone?ïíJÝ_Ë?i,o°š'?bµ"ù 5ð?i,o°š?ït³	ùÌÖ?¡!f¶Ý¾?'ižÀÆe3?¡!f¶Ý¾?î:M/þšÇ? 'Ö¤W¢?¬[-Sœ? 'Ö¤W¢?ìGî!˜?°žµX¸ƒ?¼ÀŽó?¦?°žµX¸ƒ3FGL J1444.0-7033@s'ÂzcsÀ#r-"ÁÀ9æÆ:"‰À;™jZÀ†<¶¿š4@
u_þmY@–­ _¿æU¶ëè=¿éDT@(4¿Õ$8܌ֿê-h(»éƒUNASNonenone?ïíTÛT ?g1¨o"§Z?b«$æ«ßò?g1¨o"§W?裡¯79?˜¼ðoU_G?†Ô2?ñò?˜¼ðoU_F?îÚ˦ž>ª?–q|¢nâÂ?¢SE–N?–q|¢nâÀ?ïÿä("‡?Ê
¿°>ëê×ÝyMÓ?Ê
À 3FGL J1445.7-5925@sÐKÛ ¥'?ÑèxD4b]À8¼~Ù$À: ^ØP?ґ£¥zè@
~p+—@»;\_¿ƒ‡éÕY€Õ¿è%D
y‰6¿éW"#žô*¿åc}äd÷"UNASNonenone?¨¯òÍóz??¶Þ€X±py?îuÓ È\?¶Þ€X±py?ÞXØÍv¡%?ÔüOòv…b?àӓ™D¯n?ÔüOòv…b?ܙ+c)?¶—'AÒù7?á³jNk|¹?¶—'AÒù7?çÂÝý­þ?Ão‡ÉK@d?ÐzEè¤?Ão‡ÉK@d3FGL J1457.6-6249@sÌn—OßÀ2ô™špYÀ9;ÛmiÀ:Ú
>¬ãù?ì^bq`@žžô@™G€r+A?ïË&´A2¿äI
¾À«½¿íñÛØŠõ¿àÆ\_SUNASNonenone?â,–&–²1?Ôìc3µ;c?ۦӲқ?Ôìc3µ;c?à›ÒºæåÁ?ØJÔÕnõ?ÞÈZŠ24€?ØJÔÕnõ?à»Õgçž?Áþ&)UÄ?ÞàˆU00Å?Áþ&)UÄ?ÍLßüÆm?Âg;mÐ¥†?è»ìÈÎe?Âg;mÐ¥†3FGL J1457.6-5355@t÷zö@d@æK©K¾DÀ9™'W«¸€À;	……`ý?ÛIÝޘ¸@
1$¢e@Y^ðá)¿ç|m(CãQ¿ëݞc­Ï\¿Üb–#S¨Z¿á灇»0ÿUNASNonenone?ïáÉÆNŒ{?wéBùÚë?n69±s†?wéBùÚì?ïsŽ­ýÿ?°^·Øf?œ1Ž*@@1?°^·Øe?íÓzÎÓªc?¨éꨪEž?±d)‰b¬å?¨éꨪE?î	TkT?¡"é-"÷P?¯j¾H	J¶?¡"é-"÷P3FGL J1458.7-2120@u)u\)@@JŸ±À9­—1àLÜÀ;•ÈFUNç?âƒJEžp@†úc
@»Å@;"e¿äËOT"š7¿à®îaᶿåí?}̒¿ïÿ°yÚâdUNASNonenone?ãȨf™Î	?χÔ~ýÎP?Øn¯2Ìcî?χÔ~ýÎP?Ì]EúXWD?Î%ÿéƶA?è讁iê/?Î%ÿéƶA?årûä!'Ö?º?5\¼È8?Õ7¼úS?º?5\¼È8?ÐvzÂ?³ê3m@?çÄñB¿ó?³ê3m@3FGL J1502.2+5553@W2>BZîc@Js,­'À9},²æqºÀ;îW"KS»À	úf9oã=@‡Þ@ª£ +²¿å9_¨Þí¿èëBó^uÆ¿áÎÒǞ̿ìOq4ÿUNASNonenone?ïþògSD9?#g
çB)? ي˼fŒ?#g
çBR?ïËãÄ4*?ŠF¤dðŒ?zåêòº?ŠF¤dð?ïËÅÞ7†V?"¸Ís§?zä<ÕI?"¸Ís¨?ïÿþkC÷>ÀarވX>©KϐŠHÎ>ÀarÞ~â3FGL J1506.4-0340@v,ï~=Á@F•´¢3œÀ:$³ÑSDKÀ;}fÿéYË¿Ùœx,r¶@
²…-Hc@ªyßêᶿà¥ÿEÅÜï¿ê^k¶Œ·¿àÑ@ÃzÏ»¿âaZÿUNASNonenone?ïü߅eGö??J…@Ö;?9ÔÕÀL???J…@Ö;?ï<錘
Õ?¤ürÃ4f?˜bÎlþEf?¤ürÃ4f?îªhc`¦?žH:·²Zå?¥YyΉõž?žH:·²Zå?ï«ÚNܲ‡?,Øm¨Ô?…	lHÓ^D?,Øm¨Õ3FGL J1506.6-6219@sÞò<ÈÞ+À¹§Áz‰3À9g´ör2À;¼(ßó¿ÔZë´æÉ@>—Îé2?ýµ¿©M¿ï»;µÀó?á<¶(Æs¿Ýª6˜K‹¿ÐQ¯ÝJ?âUNASNonenone?Šeò?‰ o]°?‰V]fƒ~9?‰ o]°?îõ›>hä?°B«µ^Äß? ¦Lq¿ç?°B«µ^Äß?ï Îwâ?'¾˜fBÐ??Ûæ1¤?'¾˜fBÏ?ïÐ?"ƒD?ueº'3S?wóà=¾^_?ueº'3T3FGL J1510.2-5754@t›'·þ?À›ý6¡ý–À7Ûx\2/þÀ9öð{þ~ ?âÍ'æxð@™3& !@'qàBŠ¿Îh›!%‹ø¿èˆÀa•­b¿é8©F຿è"x±OÚUNASNonenone?Ì#'ð?Ì8Úõ¡ ¶?è÷:¾xv?Ì8Úõ¡ ¶?ߝJŸsÉ?ÔsvI€þ?à1|Z°F?ÔsvI€þ?َªO‹‡w?¾_í[IíO?ã8ªØ:<F?¾_í[IíN?éuþɇ,:?À;ñˤ‹?Ê(ÙãO?À;ñˤ‹3FGL J1512.3+6622@Yò¬![š[@F•ÿŽÀùÀ:ÏDÁ~À<,)d}XÀx½VQ@Œ©-oz@Ô UŠ÷¿ëÀK÷œ¦Œ¿ÔÖr@Aí¿æ»™i{¢@¿ÙL…Ç2UNASNonenone?ïË9ú*?ŠÏ6½Ÿš?zcüj¿1?ŠÏ6½Ÿ›?ï»z˜gh'?•Y<-±B?!Yæ%Û{?•Y<-±A?íVÛõÊ3?¬8×BûZ?µO9 Q®h?¬8×Bû[?ïÿߛµR?˜ýbÙ~—>þ02%Vʔ?˜ýbÙ~3FGL J1512.8-5639@t‰ÞÒ?ðxÆj²üAÀ8«l)ôÆÀ:y*GÒ&©?q»I*ß@X"©Èeà@³J'Á¿ä7hˆ:ݳ¿èc#ÿõªM¿ç®Â¾+g¿âb¨ÄYážUNASNonenone?ïDÎ?ŸJóäéJ?—f<~?ŸJóäéIÿ?ëδšUh?ÊèÁ"^A
?ÀÅ/™–ª^?ÊèÁ"^A
?êÐ
êÊ|O?±Œ'ÄK?Ä¿ÈTÖÁ?±Œ'ÄJ?ïÅôþ
\?u4‹z¡?}ü€úÒ?u4‹z 3FGL J1513.3-3719@t½Ï€Ü3r@1u)wȎzÀ:Ž»üÊÀ;¯=×Ñã?'{,¤ë@¨>?úõ¡à:õ¿ï£ŸB"¿?Ə`"¯ì?Ô?~~¶¿àMÔ)–UNASNonenone?ïüÖPCºƒ?:¹D
Uv?9M}â+ëh?:¹D
UT?ïƋê?<Ó?….àãñÏ?|º
àa–˜?….àãñÎ?ï¹³Š€9?{C¿¨Èb?"_þñé?{C¿¨Èc?ïÊ>ãfø?†'en?zàŽwLƒö?†'en3FGL J1513.8-6250c@sædobÀMݤõîÀ8SŠÁ'À:Ü»ÛãÁ?ÜA¿¼Ý°9@?' *læ@¨V¿ªOt¿Ôîà·ª¿é"K"W¼¿êª{GZBÓ¿ãìÕò]UNASNonenone%?ì?<H€´·?¿CsÎòzP?¾»úZD?¿CsÎòzP?écŠ—¸P?ÍçV¸¬Ž?ÊqÕ¡öÁ?ÍçV¸¬?èJÖP$§…?·¢ää-\?ÎÔ¦¿maï?·¢ää-\?ê
‰wüˆ©?±Î¬&Ã?ÇÕÚ 
Ý^?±Î¬&Ã3FGL J1517.0+2637@DD¾´ .@LÓ!ž¶9À:֖»˜ÇãÀ<®U¿ôŒ•YîÞÅ@
Åë Ík@ÄÕ"?ïÿ‡à'/ ¿ëÿe8Çz[?Éc G†¿äO€ڋkUNASNonenone?ïþV¤Û×?BD(þª?&*•²Bˆ	?BD(þŸ?ïµw>æu?"
!Æý?'¼â0FbÓ?"
!Æþ?îÿèÞ¨?–°£A–? ÑrUr?–°£A—?ïüÝo‡n
?DÙ¸lç³?9ƒÄ¨?DÙ¸lç³(3FGL J1517.6-4442@t‡JB®Ñ9@%›î=_ÜßÀ9^dµ—&À;=_0Ϭ?ßÓ-‡ç@C÷¾½ë^@²m¹¿éBÚx1¿ä[/Õ@õпèhÁú®(ê¿íÿ:Ó*UNASNonenone?âuÚ­?̀ŠqûŒ?ÛÞKÔ¥Ë?̀Šqû‹?ë9Xg•L?Ĩt(A?òžaªÓ?Ĩt(A?åaä14²?¼"d2*ÝÏ?Õ<6坖Ÿ?¼"d2*ÝÏ?ä‹ÖI使?´ný÷àwq?ÖèSl6"€?´ný÷àwq3FGL J1518.2-5232@tEš¿4@‡;…èíÀ8ÔÜޒÇîÀ;ëÚ¯
Ÿ?ôèøo"@ŠìËÅ»¶@îÿ´€¦¿Ý;|Râ¿áhʧ·?¿âōñÎB¿îìӍ†:íUNASNonenone?'Ãbصe?"$Q®ÅñÅ?ïqäé:W…?"$Q®ÅñÅ?ÊQ$uý»}?Êíù"ú±?ék¶â€'!?Êíù"ú°?½mc<''ñ?¯È-þ¦‰s?ìRS˜mÛ?¯È-þ¦‰s?Ê8"¶¢Êj?©ÂÌ$E¡z?éq÷RWMd?©ÂÌ$E¡z3FGL J1525.8-0834@v,)³ún@C%žYò»À:©Yš¦	À;²X'hLð?ªf€‰@À—µ=å?úM]ÞØh¿ïÿܬhÔ*?ïه2X&?ßÔUq{¿Û†fÍz­×UNASNonenone?ïúᩃ_?N#Ñaa€?GÜyYò³?N#Ñaan?ï²f F'?–̸{Hiü?ƒy¦Wî[~?–̸{Hiû?ïs½ã?‹²Hün•g?ºc9‡?‹²Hün•h?ïñü·Jª?u¼cÈʊ?\'kà­Y?u¼cÈʊ3FGL J1526.3-4505@t˜Éšé$ò@#Bö@c^À9•xgðª"À;FKMÜ?Ú…`I
]@¥Vôƒu@#—Á¼M¿é—Gý¿í[ÌçFB&¿ÐG#H•¬¿Çh(ˆ¤UNASNonenone?ïþ)ñ_I#?1U¢\Å£ô?-`êmӇ?1U¢\Å£ÿ?#«Ëa'?•2é4‰?€ß
'›Å?•2é4Š?ïgCJ²v?ŽÇïÛæ‹ä?"–©±/Î?ŽÇïÛæ‹è?ïÕ¦^ÛO?q¹øvâǸ?uu¬Ð'X¬?q¹øvâǺ3FGL J1527.0-3804@t܃ä%¯@.¤ÎóÀ:š'Í¥:À;€¦'F•ç?¦oÑòlÎ@6žK…@¡í`@1ž¿ä†¢Æê¿ì'Vv{ª¿É€@›ëGP¿Þ°4|UNASNonenone?ïþ»Pá?5)|¼îá?$Oêþ'ça?5)|¼îÌ?ïÖóbl;?~}ý¸t?t†wNÉâ?~}ý¸u?ï¢#|?…!Aåòy?‡{· ß¼?…!Aåòw?ïܽ¢°#?hÿ‹¹%?q¡.¿'îò?hÿ‹¹$3FGL J1528.1-2904@u9ßý`é@6m
$F0fÀ:ˆäö=öÀ;¡míCdÚ¿ë;
ª‡½@
–cî<D?û%÷@=ݱ¿ëΜ¡n¿ÝÑäy;Ö¿¬¬àÐ
?¿èº³Î,UNASNonenone?ïó"œ	eª?a?Zƒ".Å?XöÇí4­N?a?Zƒ".Æ?ïՒ¨×`?€?­ƒ9¯€?u6«"Ïê?€?­ƒ9¯€?ïÕ«\-?–¹É¤H˜z?ž%J"z_¨?–¹É¤H˜x?ïúd—Ðõd?Sïh³¬?Fm ¼*q?Sïh³ª3FGL J1528.7-2247@u€Jßø"¼@;Evš'^À:™ï)îçÀ;šXKñp?èÁǒ-ù@
ێ	Ãx:@ðßëb¿Ùz£QJ¾¿â-J¹6Âà¿â™3ÅÕ6Ô¿ïÿÆ×âYUNASNonenone?êù앇‰?Åõ+'B•?ÇÀM©áÛ?Åõ+'B•?â­Møé?Ì&oEU˜?Ú¥eçÚ.?Ì&oEU˜?åJÛ¬R•?ººê8}Ý®?ÕjH§ZÕ÷?ººê8}Ý®?Ûa$ϒ.
?¸:šó9±€?âOm˜6èû?¸:šó9±€3FGL J1529.5+6733@Yß1)Ë«@EŽ'_ét£À:ÄŵV­À<3r"XÀ¿ëg¿p³@;P'¾N@å
ŸÁ%û¿ÔÌ!nî'ï¿çnéÍíî¿ây|ˆD¿àÕõÀêtUNASNonenone?ïà±W/è¨?ÝR³ˆt?oN¨ÐV¾?ÝR³ˆt?ï¢Âææ-?˜mdg{!?‡OFFxôî?˜mdg{!?íÒð\Øßp?§Á®N
?±h}9'?§Á®N?ïö?ɱK1?R…ƒv±Ö?S€liŸq?R…ƒv±Ó3FGL J1532.0-2618@ucblvK@8ºˆ&«À:#Š·~‡À;†@Ú»¢Ù¿Øp™Ã@ú¯Åüe@uí οௐæº9¿â(GŽMÏÛ¿àç¡Ú…È¿ã¥1 Ö²UNASNonenone?ïù~ACÑ?P`H©/è?Jú󰽝?P`H©/ç?ïÊ·êµ·T?®®ç+ãN?z¤
¥$V0?®®ç+ãN?ïŠ8fï?"£ìôûùY?œn¸ìS":?"£ìôûùX?ïÌ[^û`?s—¢¹Ùr?yÒP'sÐX?s—¢¹Ùq3FGL J1533.8-5231@td <K	ê@"]¶ŠÀ9m'Y4À;
Vìu߀?âÎApQ…@KšÌ>‡?ÿrû?{ëß?í•ï{«ûz¿Ù˜Ù]Ý^¿×(>;é©ì¿åŒ2 2²UNASNonenone?ïv5ìé=]?'ÁӇxšë?'9BbØTV?'ÁӇxšë?=2?¾£\ÿíÖQ?¯T¬/Læ?¾£\ÿíÖR?î°÷94<i?™Å:kkM?¤ðŒl¼9q?™Å:kkN?îSý)¤Z?›,m'-¼?ªÀ-e¿ªa?›,m'-¼	3FGL J1538.4-4656@t¢þÅm\û@¢—žÖÜÀ8•;!>>)À;còPë?ìºO¡þÂé@Ë­MÖw›@˘¿Ô쬿èo‡]"V¿êúÌ5¼ê¿ê"Îà¿ïÿ¹€Œ#ÝUNASNonenone?ïÌsô×Å5?,òO/¦@?yÆ"dú?,òO/¦A?ác%§‹Ef?Ò¤®›ë?Ý9´°éu2?Ò¤®›ë?ëÞQÓúT\?­=*ô¢‰?À†¸°®"?­=*ô¢‰?ÑÎeghR‹?±ƒÔáج?çÍLKÖº?±ƒÔáج3FGL J1541.6+1414@7­ ÝD@H2`=WyÀ:eøg…JWÀ;¯ëí#"j¿ß±‰ñ—Å@
#Ïj¶Ø?ÿš¿5Š{¿ï §IŸ?íx‹dw£Ð¿ãW}vö¿ÞÈfžùœUNASNonenone?ïüWÏ	ƒ*?@»¶"ÇÉ?=A‡³æ®?@»¶"ǵ?ï7ÍX"5?¢¶	þ?ë1?™Tý™X?¢¶	þ?ë2?ï‹]É/4þ?†ªü8
4î?(´2À?†ªü8
4ò?ï—$ëÁË?Š|c:KâO?Š6ō?D?Š|c:KâO3FGL J1542.4-5911@t4ÿ'+¾ËÀ
-\Äüô³À94If{_À:蟔…]¢¿ë—7'js@2·7dE@Ðà©-`¿æq-ãÀã¿å¹û6(¿êdV#Ö§u¿è¶u>_PUNASNonenone?îÈríÅ?ªö«¸y®•?£˜Ñ#Æ?ªö«¸y®•?îÔx~"'?³#ó\D,ü?¢¸xß͇?³#ó\D,ü?ëå(ŸP?°ÒMTPó`?Äk÷]'Å?°ÒMTPóa?ïÖEM†þ?tœkê¿y ?tÝY<ûh?tœkê¿y 3FGL J1544.1-2555@u‹ÁÝ!ê@6œŽ:!dÀ9/Ô!Tä^À;Y 8ð?õ'ÏÐã1é@qɎ~ÞW@Þ]@L÷*¿×Û«Ë(œ¿çêeÜJ:®¿å¸y™§¿ïÿ§¿!>UNASNonenone?Ð!w
R&h?Åõ¥
öK?çïDyVìÌ?Åõ¥
öK?¹€°tN?»3o7aW?ìÏéþ¶?»3o7aY?Ør—™¯?¶ý"67<?ãÆ´3wò¨?¶ý"67;?·Ááµr‡x?™1èÄx É?íÃÉQ¯?™1èÄx É3FGL J1544.6-1125@vC`¿]x@@~Àð¸À9iW²n}À;Jǘ°eŽ?õºçG!}@á—YÎR‰@M`@1ž^¿Ájàܷ"¿çà–>¿æ	`m?¿ïÿá&Ž4UNASNonenone?É­{ø½?ÅÓF'¶?é½Ô¡?ÁÑ?ÅÓF'¶?¤—D"(?¬M>°qè?½ßÝ?¬M>°qç?Ԁ	EÔ?´p{r؄Ä?å¿ó{]9?´p{r؄Ä?¨¨hyuv¨?ŠKaN!%[?îuyxh¨–?ŠKaN!%\3FGL J1545.0-6641@sîἩiÀ"Á'Ýãu†À:'Ns*šÀ;r3#Bû?Ñ…cñZå@ûÉTrH?ú¿æŸÜ©º¿ëÖ€BÓ¿å"x†/Ú¿ª5.é€k¿µ\]è­AÜUNASNonenone?ïþÎ>°²§?&
j–:o-?#ôՋ¿?&
j–:o?ïYnÃj
?¤¥?*)L?"Ò''¾^þ?¤¥?*)L?ïÜÖyž¸¬?v/Lœäù?q"Ã0£©ü?v/Lœäù?ïùà'áDz?D{$څà~?H}´xá5þ?D{$څà}3FGL J1548.4+1455@9¡ë¦¬§"@G–a©É"À8õªõâoÌÀ;g8¿E%?Ü26Âù~ @Ø"´Šá›@å­_Ÿ!ï¿Î¾¬ÒË-T¿á™n·©á¿ãJŸfy¿ÝT{eY©UNASNonenone?ïö1?ZpMbÆÚÄ?SÃÉáï×?ZpMbÆÚÁ?ïZĬ¨pü?šBÚòÇg?"§jjñà€?šBÚòÇg?ïNðu	S+?'&S%¢?–!ñ^՚"?'&S%¢?îÉC÷mÊ?"º©Ñ?£kÀ‰#`?"º©Ñ3FGL J1549.4-4832@tªó¡LìB@ìúi¾
À8²³8§{À:ÑuúÔG¿é1©´€@~A…†g8@ïš@]".¿çòŒEYa¬¿íc\‰ÿÙÑ¿Ó«›q,Šo¿èp³hÅUNASNonenone?ï|Og)éæ?š.L†"§?vÂÃ"?š.L†"§?îÓ¥ˆîôç?¶ŸvDƒS?¢Å§q±?¶ŸvDƒS?ëÒ·±§"l?°l_1K3?Àµ!9cvR?°l_1K3?ïVv(?šOõ55Ü÷?•1=Zý^9?šOõ55Ü÷3FGL J1549.9-3044@ueâ'@·€@2$<µ¬À:f6ýÃÞÀ;"¹
Ó'Z?éÞ~š²Ý@€n1áÏh?÷¦¿òÉ·¿îm~ÂÂ?ï÷TYb`·?»áéû—÷"¿¡Å«%.ÏUNASNonenone?ïù%b¸?O¿ôë®\:?Kkžu"?O¿ôë®\(?ïÉUí8»e?‰{ڗu\?{U	c¢M?‰{ڗu\?ï‡RØn1?"(hۊ»
?Ï¤ò9Ú?"(hۊ»	?ï4LjÁ€Ê?—ÜâÉl?™vr§ÏæÓ?—ÜâÉl3FGL J1550.4+6027@W^qŸŒ¨@F‹ÙÂ~•1À:TcûRÀ;ïèwM>w?¬cª²h@jùÀöªÂ?ýƒ˜ Õú?'Wÿɸëû¿¼!`DZÅ@¿Éb>ÛÕJ¿çW
×ÈÃUNASNonenone?漣(´%ä?'k'ÕÈ͂?†[uÒö†ã?'k'ÕÈ͂?ï/ðð)2ö?¡q¤'ŒÐJ?šáúÙ¡5?¡q¤'ŒÐJ?îˋ˜"ô?™sl¹sIÞ?£GFx°Ó?™sl¹sIÞ?ïD×?"ï7:ãÀ?÷½å?"ï7:ãÁ3FGL J1553.1+5437@Ue3]$žE@G•¶Ü gÀ:&¤¯wÀ<y_gn¤¿åZ¢ÕF\Ê@˜•¸Ž|@
eÿ¹3=¿Þêø˝¿á÷d¾¤µ¿ä]ql¡5¿é©Ïzã1NUNASNonenone?íÂi<(;[?ºhû"w6"?±ì¶¾%'?ºhû"w6"?ïè6þ?§äÞ²D'Q?Ÿ'ð> N?§äÞ²D'Q?ì"FñtVÙ?©ùùhÁŠ?»eÈt]I3?©ùùhÁ‰?ïÄÌE ?zØu"?}ýÝ/±S?zØu"3FGL J1553.3-0322c@vñýÞ½@BJ^Ý)5À9mlÓgñÀ;Q'TPº-ÀYsä©7@Zž¥òîJ@€p]¶¿é2ŒÚø¾¿ãå×;K줿ì2©J€q¿Ä?"úÐÐUNASNonenone!?ïōè'?'ì{È?}9ú|·±?'ì{È?ïÓ»ò?ƒ¤¹k&'?v"¿9?5?ƒ¤¹k&?íà@†ç½? 'Ô³w~Á?°ýûÈÇ¢? 'Ô³w~Á?ïÿüÆy>Ò¾$	wé>¿YÌ7{1>Ò¾$	sÛ3FGL J1554.4-5315c@t"Ùè>B[?Ö-íCdٞÀ7Üݸ­[À9Øró<£?òí±ÔxèŸ@76³t @
 8ð?ÜÖF±rÜÊ¿ÞGh¤¯!k¿åZeCё¿è°Œ'ãRUNASNonenone0?‹¬<×0ô?éE‹Ž?ï¹ÑO£;?éE‹Ž?²ÖäØ=—?¾¦•D<0b?í¥#gŒøN?¾¦•D<0c?Äî‰ê wÏ?´ÚÕçâvX?êÄ]…wâ?´ÚÕçâvX?Ív@#X	?¹p&꽖§?è»âo÷)þ?¹p&꽖§3FGL J1602.8-1924@vç#$È6@8Oh7÷¾À9Þ_>Sø¦À;eéÁЈ¿æcÊ«Æ~@l˜Œ´Y@€õs}¦¿ãþö,RÕ¿çIQÈt£k¿â6©µF¿äžÙ—UNASNonenone?ïývH¬I?6YL¹M?7ŒMº·?6YL¹q?ïЇÁp×ð?€ì¬÷Ÿ?w¼G"T?€ì¬÷ž?ï"Å ¢td?…î…¾/,Ÿ?ŠÎ—×bæÜ?…î…¾/,?ïæ²zÆEÍ?d̜›Ùï?iM…9º3Å?d̜›Ùï	3FGL J1603.7-6011@tLƒùdÀùà`þG™À9è¹/a›À;k½"J¥@?ôèâ'Äb@hScTc/?ÿeþ>´Æœ¿äتÐgzÒ?äÖ©G¿Ø&ã&³ü¿ëMãÃçÔnUNASNonenone?´R-&â"?µÑçÀUw?íuº[#­?µÑçÀUx?ÌÿÉüÕå?Ð:—›7s?èú€
€Ê‡?Ð:—›7s?͚.jã²?³§©"wå?è™t~eG?³§©"wä?Ùý­oc?Á#@MP`?ã})uHN?Á#@MP`3FGL J1611.9+1404@;ÈnÁ~ºñ@DфV!uÀ9ÞÊ#¥ ¶À;¨÷ÇLZL?â~M±A^£@5»Gdâ@­_á'¿ßTû‹bZy¿á˜'xñ‹ý¿æÐB=šÈÌ¿àÇB+@UNASNonenone?‰½0?®Î'P¬?§g‡d,÷?®Î'P¬?îšãȐ²è?­ KÂ-S¸?¦QÃvôÑu?­ KÂ-S¸?ìÚú ¡°'?°#Õ1¦g?¹(.úò{h?°#Õ1¦h?ì=P;c-?­)€2ã-?¾…~$æ–?­)€2ã,3FGL J1613.4-4222@uû_ïJ@t‹e#pHÀ9p¦]¨À:óˆBY@ä¿ûÚOÊB®Ñ@cƒ•vI]@zs 
Ìã¿â,3_%ª¿í— m‰¿Ûš+ošl¨¿åÁü¸‰1UNASNonenone?ïõáȃô–?[àyµ_–?T<nøÕ¢?[àyµ_–?ïÍÐPv(?ˆ_ð§¢?y×Äÿëþ?ˆ_ð§¢?îQÌՃ;%?£al'±«?ªã2§ÌM¸?£al'±«?ïþôFø?,w;^⁾? ¾þ{Žß?,w;^3FGL J1615.6-4450@u*™0¾@?û¹IbÀ8Ó%žõùíÀ:³ËE
PK¿ì@†÷ð*å@Æ4/²u3@~ó€jÉx¿ë`ûZ©Äµ¿çÒí!mc¿ã"T
"¿äÝ
ë-¿UNASNonenone?ï羘ïbÚ?rÁWÃjV?hAg&&?rÁWÃjV?ïÃëá
¡?'=]µïM?~
zý¯5?'=]µïL?í)‡­HV?¨¥\¸Aµ¬?¶·+•½J?¨¥\¸Aµ®?ï÷17ÐÑ?RúU`G?Q^xÜ´?RúU`I3FGL J1616.8-5343@t§—¢H"ÄÀ½Õü woÀ8ZÉX¤À:ªí"Ãq?äèKË@]ÄKžäÝ@=Žà-&Õ¿æÔ¾+Qðì¿ãy9Ó>­¿æI"܍¿ïÿÍݐ`ØUNASNonenone?Ñ	«;;ˇ?Í®ÕÏð‡?ç{*bb<?Í®ÕÏð‡?³9iÀã‹?¿ñj¿ÛŸ,?í˜ÒÇãï?¿ñj¿ÛŸ+?ÚÄ-•É?º5HÞÄÏ?âðiv5?º5HÞÄÏ?Ô×½=òf?º¹'Ÿ"?å"!xaÍ?º¹'Ÿ"3FGL J1616.8+5846@Va
xÀ@EX¤Ò²ÀÀ:1ùˆºWÀ;ÿ1æ,?Ï¥#\óÃS@ǐ:`˜@ʅ˿î'ßÞCå¿âÆm1ܛø¿ïü"±Òæ?ïژߛSUNASNonenone?ïÇÏÅ\´î?‹¦"€Ø€?|Q¥‰Z?‹¦"€Ø€?ïœÿú°p+?–2PˆâÂ?ˆÀSãõ%?–2PˆâÂ?îo—l€*P?¡žå8o¿?©‰7ý[?¡žå8o¿?ïæRÓtˆp?w¦THÙ'?i­,‹w×?w¦THÙ'3FGL J1618.8+5520@U:rŸYÌû@E¹¿ðEwÙÀ:·!†b…0À<(‰hÉíõ?Ûrv¥"ä±@n@'â@œ?ÿIw¿áðÁ?·¿ãô™'ì3ù¿ãQ厾I¿ïÿo•þÉ8UNASNonenone?ëǦ~?Éõ6µv®:?êàÍϲ?Éõ6µv®;?ÞeÔVñ?ÒêÑêOxÄ?àÍz÷Tˆ?ÒêÑêOxÄ?èZJí¯¬?À½®¶ÇÚ?ΖÔIA‰M?À½®¶ÇÚ?ÝêÊbÐã?Ä×sI%¿?á
þšÎ—?Ä×sI%¿3FGL J1619.0-5014c@tÒy»­À˜?Ÿ¶a-ºÀ7á€hp+âÀ9©{rg%©?ñÂC@–ÕU‡pø@s|‹5©¿à2׶=r¿é'¡˜Êr¿èíçؘ¿å²8]$ÚUNASNonenone9?ʺ>n¡ô?Éý›B¤›ô?éQ\°dWƒ?Éý›B¤›ô?Þ½#åæS?Ó绲ÎN¦?à¡n
Öu?Ó绲ÎN¦?Õ6ÛOAð^?»¥+.?åd'X_Ñ?»¥+.?äÑðä?ÆÚۖ¶À?Ö]þ7×ç?ÆÚۖ¶À3FGL J1619.1+7538@[EÐ|"µÝ@A¥ïÝëÙÀ:ԛÀ»F"À<%ZÞrç~?âÀùɞÞÂ@~¨Q˜?ûg€)†¿ïõÜíù›?îã†tù§ ¿à"m¾‰-?Âs¿Æ»!UNASNonenone?諭¬ûX?''öz¾Ê&?…PTø*?''öz¾Ê'?ï»Ó†%uØ?Ž?7£6]?v¢‰×?Ž?7£6\?îœ##y·å?¢¡åòSº?¦=ÍÈd¦?¢¡åòSº?Bêru?ŠÊgiUÄË?¯Ecbã?ŠÊgiUÄË3FGL J1620.0-5101@tËa\¦Ê¿ä?ØÝý ÓÀ7çÇj<"À9Éb¯ø€°?ñÖþí|l@_†`ÔV@[€YV³¿Ôꔉöt¢¿Ü{õv[žY¿çÎ3¹¸?n¿ãf1R2|ÕUNASNonenone?3ÃÛ aj?§ •²Ík@?ïaá"üõ?§ •²Ík@?ÐY*.9*ã?Ψΰán?çÓjèãjŽ?Ψΰán?Ðâ—É Í?¸™|['i?玴|¯›?¸™|['i?Ú(ç½j˜š?Äþ‹¹jùH?âëŒ!J³²?Äþ‹¹jùH3FGL J1620.8-5149@tø}¿H¿ô™@
6IhÀ9
Ñ­ÝÀ:oê3åàš?à¹+¤bd=@™Ä6%@»Õ@Ž»o¿ÞmW°¯Ï€¿í!]'澿CD?S)üT¿åµµAüàÍUNASNonenone?ï3òòG3m?¡]'êe™S?™¡·'}?¡]'êe™S?è,¾YSs'?Ñùi#V?ÏMš²1½?Ñùi#V?ë0Óí(•ƒ?°Mä"¸$t?Ã<°K]©÷?°Mä"¸$t?ïsƒÿñš?œ|–•e ?'€ßìÇ?œ|–•e 3FGL J1624.2-3957@uQ¢3œ¿@–ž^$x…À9 €©ÌÀ:³À~à°¯¿ª´‹P‰@×´>ág9@(‰ðü¿ç"[À×1f¿äEmG¿æ?d€¿ïÿá{ýɼUNASNonenone?â ¦Äð?њØbñF-?Û;²vÅ?њØbñF,?æ˜!©?Ðþn´~Ç?ÓÔϼ­Ïü?Ðþn´~Ç?ã…Éh"J?µÊ'¥>?Øôm.÷jþ?µÊ'¥>?ä¿°¦kY?Äå:®Äò?×Ҁž³)L?Äå:®Äò3FGL J1624.8-4233@u4®}Vlô@…`&±EÀ8ËAøÈÔÀ:¥Zs¿èʔŒ6@2ˆ9tëº@:×@H÷¿çD"8­¿èCÂöÆV¢¿æxþH𴳿楿l¼íUNASNonenone	?îL…¬¹~m?­©ÖÙt®¹?«7¥4h1?­©ÖÙt®¹?ï³`³Ø0–?›ÁƒŒ¾?ƒ'Ó	óÚ¢?›ÁƒŒ¾?éôöÚùÂ;?²¤Tԍü?È,$"÷?²¤Tԍü?ïÝ«Õù6?r©•Ô/?qvªdì?r©•Ô/3FGL J1625.2-2845@uØ_ôö@,fÃb(À9xx·¡ÂÀ:ê$=Ìê)¿òôv	³@ÁþÙºF@)¾×ü¿êÔ½âvá¿é¬ë';¯·¿á»<QÈ}:¿ÓBBÏ»óUNASNonenone?ïûpõöô2?L«v_HW©?B<($/6œ?L«v_HW™?ïáÄBçw˜?x˜kXÇÝ	?n;½ˆhÉ?x˜kXÇÝ?t4?¢»#),Á?¦çîH¼¼?¢»#),À?ïþ­QÕÛ?'ÕW:ä9?%*çâ¢=>?'ÕW:ãä3FGL J1625.6-2058@v:®záH@3I§;BÌ-À9EÓ)Þ À;"Pg÷`?ÓXŽ-ø@
g%Pq‡'@SÏÿ²'Z¿âž¥ñQø¿ìáWb+]¿âøLòì¿ç¿ˆOªUNASNonenone?ïÊÅA¯@=?€ßè5õ"?z_(_ád?€ßè5õ"?îŠø5Ú?®úËמ)t?§^>|¢c?®úËמ)t?íåù£`¤?¢!Z6¾ïq?°Ð2çôúÚ?¢!Z6¾ïr?é|oÍN?µ
ápÙ*2?˚@ÊÇ«?µ
ápÙ*23FGL J1626.2-4911@tër{²þÅ¿«Ýqà˜ÆÀ8|‡5DÀ9×ôm$Ɖ¿ðÞ	îkX@PæMÒEÞ@ÚÁ`ˆ¿ç%—=$¿é«´x÷¿âì7È]¿ß¡Ìts€'UNASNonenone?돘ôöù?ÁßZ$µR6?ÁÁœ-¼$?ÁßZ$µR6?ëM whAã?ÐH¯éæéN?ÂÉ~"^øt?ÐH¯éæéN?å퉠Ý%?µs_"À5ø?Ô$ì¾EµÇ?µs_"À5ù?ïñaG×Ւ?ohKôd‰G?]=pPTÛF?ohKôd‰F3FGL J1626.2-2428c@vð†nD@0ä^	}À8Y
×ÊVÑÀ:]$
üB?õ¡¼Ö_@ÇWC]ͼ@3õ§:A?ïüçEا¿ç@Îk!P¿ã¬¡gT‰*¿çÒ^ö@ʲUNASNonenone ?×,‰ö?ÏV^¾S"?äviþõ»?ÏV^¾S"?ã×oHŠž¦?Ñãâ'Y?ØQ!nê¶?Ñãâ'Y?ÚصÆ÷­9?¶QÁµ	n?ⓥ")b?¶QÁµ	n?Æàž.R?´#øo<h,?êGØty«\?´#øo<h,3FGL J1627.8+3217@Jz©?)
»@EšÙ¾L×IÀ9ÆñÃ&ZÞÀ;ÐÈ1\™^?õc\†=Ç6@úË²@=?Ñ|4?ïߞÎ.C,¿àã­±K	¿âÎ"žv´N¿ì"äΏ£UNASNonenone?Š"Xt"9?œmZéáj?¶ž/w?œmZéáj?–mr=?©ÓӫȖ?ïOܗ"n?©ÓӫȖ?ÂvšÖÒ;í?¬8
¯"Ú?ëbYJKq?¬8
¯"Ù?ž^æÜ«´?"`úÝLO6?ï
É*¢?"`úÝLO63FGL J1628.1-3344@u£"úÖËS@$¼[òoÅÀ9ÉÔQüLÀ;7ò<ÈÞ?¼Ií´ÎÔ9@Ùéù-}è@îÉÿ½åÔ¿ëõŸûø"U¿ãg€¯è»k¿à)«[I8¿ÓÌȝ4¦UNASNonenone?ï÷
á´?QgR˜œ?Qê=ÇޘC?QgR˜¢?ﳋÔ|?Žâ;·:)?ƒ=Êàܦ?Žâ;·:)?ï‹&meÕ¸?…›²…?6d¦Š'?…›²ˆ?ïpæüq?…¡gÐ
ž?'ã=žàr
?…¡gÐ
žŽ3FGL J1628.1-5740@tŒŠ\å´$À"yÔØ4	À9²¥ùú,À;#áâއ	¿ÚS'nGË
@×qýÉD@¶ RÛÅ¿å@+=U¿éÐb×CPë¿èV™µ{Õí¿Ô۝Fï UNASNonenone?ï•ÿåº×M?Œ¸TÎ/ài?Š€'J,²?Œ¸TÎ/ài?îÞ؈ÊÌP?±ÂÌUÿÝ6?¢wsS;?±ÂÌUÿÝ6?íí&z]V?¡¨ÌÙûË"?°–Ì-Oé?¡¨ÌÙûË"?ï©äÆònà?€!®ρ^?…†ÎCdGè?€!®ρ^3FGL J1628.1+0254@1¥‹'¡¡@@t<òϕÕÀ:L(Àª'À;´Ì3?æ"ßÉ\]'@M÷Y¾7@ú'ßk5¿º["'0®¿ ÷?$‰ö¿êP*v˜…¿×b2¢ó9UNASNonenone?îq¥M}Ø?°¡l)²«?¨ï5«("u?°¡l)²¬?ï~bl'8É?™
Á{âˆ?3²{æï?™
Á{âˆ?ìb¹;?°Ítoz?¿\ï6'?°Ítoz?í`¯eêÕT?¨s4wE½Ã?´ú"ЩUc?¨s4wE½Ã3FGL J1628.2-2431c@v(C€ˆQ@0ƒ	"ãÿïÀ8wÒ<çèÀ:dVè'?âöZ'@H÷¿>Ä·@ú`Ãd¿çp^{¥+¸¿åM#"qÑ¿è@Û¾hl6¿âUQ©üúMUNASNonenone0?Ü5×±¸ÓÜ?ФÞö´8?áå'#–?ФÞö´8?ê²åEÉ?Ë
Ó>Õ¯p?Å4iÉÊèß?Ë
Ó>Õ¯o?àï´âK*1?¾ê~ðÏ?Þ –;i«Ÿ?¾ê~ðÏ?ÒÂS;.ÆI?¿B¤!F¥Ù?æžÖbhœÛ?¿B¤!F¥Ù3FGL J1628.4-4546@uô!-w@kOÚ2æÝÀ8`É{ßtoÀ:aùӖª?ôxËéM!@ª˜zµ©@6 %#ü¿åî_ª¿é'*u°—¿ë9hÐ調îà#ñ÷©šUNASNonenone?"ÂnD0H?j·Æö1®?ïaìßî~?j·Æö1­?«y/U•Ã?¿¾÷Y•Q?îHm
¦®"?¿¾÷Y•Q?ÆQ¾v:?¹íriô®?êkbq`;?¹íriô­?³tFn"u? 5™-?í'w>ò-'? 5™-3FGL J1628.7-8056@sm‡~äâmÀ5ŸVûW÷À9àÁ3;–¯À;'yLò÷Ú¿À¢XÕâ©@ÿ‡Š#@»ß"¥"¿àzò ­¿êððØg,+¿çúe:í<¿ïÿ€
HСUNASNonenone?ïUJÿ!d?£,'ç?•V Ó|P?£,'ç?æªÚ¡ò¨?ÏИ@Ö?ÒªJ¼ή?ÏИ@Ö?ì]Õûb?«Œ?µµ"{?¿m9P$ò?«Œ?µµ"{?ç8ª¬wÔN?½~ ò×ùT?юª§Wc?½~ ò×ùU3FGL J1630.2-1052@ ¹™aÝ@8È!~|À9ºV4¿û-À;Y¦ùÔlÔ?òz(»
-@7î-ð~@a« §U?ïRÇ:f®5¿åIøopƒÔ¿å!'óˆß¿ïý…¿û‹°UNASNonenone?Ö7}x
x?ЋËÜ"?ääÁCùD?ЋËÜ"?œ¦êk@8?¯á
\»²ù?ïȬ¥ÿ?¯á
\»²ù?ÔB§½þ´?·òPe¥Ôy?åöÞ¬!¦?·òPe¥Ôz?¥väÞ½ï¹?"=ŒhY»?²!?"=ŒhY»3FGL J1630.3-6126@tcGd­ÿ'À!Í_™Ã‹À8ÿXz™À;\l <K
?Í´#¼%hM@–)€Výh@I`p-:¿éÀGáɒ¿èTia¿æ¯tҏڿïÿϲUNASNonenone?ïü±'Œ·¦?CÅ'Òë?:skšBВ?CÅ'Òë
?묚œXø¤?Å,ãäÚjÞ?ÁM•Žœs?Å,ãäÚjÞ?îÇΟ§ó?œ$.ï?£ƒŽÏ?œ$.ï?î›Ð˜=R?–:¸f½Ô?¦Böx*Ö?–:¸f½Ó3FGL J1630.3-4346@u2SâÖ@	†×:ÇÀ9ˆ³c$"À:ˆpSO?ðrD˶ø$@
mœ@Ô@P`j£ã¿ëA2'^>¥¿æùdÌÍ…¿ë|[Ñjžã¿ÜœJ°jUNASNonenone?Æúl°²+H?ÈË~.é9?êAdÓÓu.?ÈË~.é9?í
ð³³$\?Æ{Ίi˜¤?·¨zbfÝ ?Æ{Ίi˜¤?Þ³ïE¨ßç?¶'ÜËæHÒ?à¦]+?¶'ÜËæHÒ?åÂQF#?ÉÔìÍá¸s?ÔÄ{ý]sº?ÉÔìÍá¸s3FGL J1632.8+3838@NÞáG®{@EldE#öÀ9àõø?A^À;áý¶z?ð[(ã#%t@.£yè@žXߕ&m¿ï̦¨1@?çJ<M§í^¿åvzÊeX¿ïÿ—Ö²UNASNonenone?ÔP÷)Ï/?ÑÞØæ¢\w?åׄ}ëh?ÑÞØæ¢\w?²Áº‰Þë>?¿£^lÇ?í§È®Ä"˜?¿£^lÈ?ßg<4nC£?¸'èoJ…?àLaåÈÞ/?¸'èoJ…?°Õ8ô?¨¨{2ܼ?íå\¼Xáq?¨¨{2ܼ3FGL J1635.3+4257@Pèñ€
|@E:ž¡@WÀ:O&ò³À;òøK֘(¿ò½Fâ½yô@-Yôèõ¢@U1\¼™¿êîÛü{Í¿àÏñ´&§x¿à$'rŒB!¿ïô'½ÌµUNASNonenone?ïvé~ðž?œ3•p£ûX?'"Ð<ì:?œ3•p£ûX?ï•5œHú?":ëÇ^?Š²¸ØíÁš?":ëÇ^?ì—˶QÂq?°?ÄÎ$!?»A¢Mqìv?°?ÄÎ$!?ïöÞXq¥Â?TÀœ"S¸I?RCO´|è?TÀœ"S¸B3FGL J1639.4-5146@tä
"M;À
ËšþôgÀ7ìú@£À:®ŽwýgŸ?ãÜzª@>`ÔV.
@ËBàO`¿àüöøoh¿äÏ>"¿äk°ã«á¿æÇ1'ý¦½UNASNonenone?êÁ^ú?';‰æŸý?ÇÐñú"î?';‰æŸý?á«&î¼?Ò»jõ¢ê?Ü©Ñϲ"‡?Ò»jõ¢ë?ä>oÕ«Á?¾VÿÁ¢?׃!ØT¨~?¾VÿÁ£?åoi¾¯pÆ?¹O
×ñ=w?Õ!,'¡w?¹O
×ñ=w3FGL J1640.6-4917@uÕ<ÝÖà¿ýX™¤T(À8Y'£Ü»À:aÙïÊþ–?ìüÞ8¿_@A9ˆâ½$@tÿÑ¿äÞ~r
l¿ç~%q ù'¿ã0¥c@0¿é›XL-'DUNASNonenone?푋QT–o?¹¢ÜoNTÏ?³s¥u[L‹?¹¢ÜoNTÐ?äã5'cc?Ð"ïϏÔ?Ö9•üû9;?Ð"ïϏÔ?å°v#?¶Ój%WýY?ԟóù¹þ?¶Ój%WýY?èÛ§¯a?¹yè•ô?Ϝ'aCò{?¹yè•ô3FGL J1641.5-2856@uü«¾Ê«Š@&ÄÝÛ
À9™­»ŽÀ;6Õü÷7?먕_ùõ@tî¹[¬@] A"ô¿âH`q"Ó¿æ´æB®j%¿ëU¿]´¢E¿ÜhW΄C,UNASNonenone?îI¬™‰?°Yð?¯{e6go…?°Yð?íßa•‰ò?ÀYÖ­™@ó?±óWk°{?ÀYÖ­™@ó?êÿ8@ôU?®[*ݏϹ?Äü.«Ÿ?®[*ݏϸ?æ\ïÿ.ê?¿ñÉĽ?ÓF £ü-?¿ñÉĽ3FGL J1642.4+8045@\oÁ½¥@?ÁP¹U÷ƒÀ:A)Ý:ÙÀ<u^Pî/?ÜíÔ¤v[@j×9bL@áz AÙ¿ÞÎÕù#ö¿åÐ×b¿é÷Ös¿åSCTF0ïUNASNonenone?îþ7åáAß?ª'Ÿ"͏? ¡ëâ?ª'Ÿ"͏?í·§˜‰Df?·åc6-±(?²BÃ;µÜÐ?·åc6-±(?ì¤Pü¨§?¯wù½M˜?ºÝxºÄ?¯wù½M˜?èe¯xÝß?¸øÖw¨Çù?ÎkåBˆ?¸øÖw¨Çù3FGL J1644.4+2632@G;Ž!–R½@C@oiDg8À:*=h@[:À;¯³æKùÔ?Þr[…?x@
÷û%$ҝ@–ˆÌB¿èmsZ›Z¿î¡·ú~a?Ò½š¡Ä4¿ê,9ÓÐUNASNonenone?ïï¹$k¶â?fX6E9Uœ?`F۔IC?fX6E9U›?ï$9šÍJ?®)6V€?ž;x̦VÂ?®)6V€€?îÅa5aU?™E€ÑáÅ4?£©ì§)ê¨?™E€ÑáÅ3?î÷(ÖõÄ?¬""çÉÀ? r¯£Ç?¬""çÉÀ3FGL J1644.6-0911@!ZWɱh@6ßpyåŸ,À9¢{…²\À;5£"ŸY¿ÕÑÝHו@
5ré×u@‹³ŸÕý¿äÈ^gƒ5Ä¿ì{"'È¿Úqì"õÆ¿Ùp9Ðþ'UNASNonenone?ïýÿÞœ??weóOz9?7ps#??weóOzJ?ïÇó2ãB%?…×(zåù?|fŽ^íº?…×(zåùŒ?ïTökè»Ë?Ž ‰SUå?•a2'膦?Ž ‰SUä?ïÏ*7)×?rÆ⪩ÞC?xjäk}ž?rÆ⪩ÞC3FGL J1646.9-1332@ÏV!tÄÎ@3ä_ö"FÀ9ý»´v"²À;R]¤öÄî¿ó²¼ökÕ@
äË+­-?ý›ÃNúº¿îå±ç‡ýÕ?ÜŸŽ%G7¿áJé&¿Õä£ÖçáYUNASNonenone?ïû¸Sñæ‡?;1¤¸Au?A°8eç—?;1¤¸Au?ïގØ	VG?z1	ð$C¨?p¸"ûTÜ ?z1	ð$C©?ï¨õ4"g??€ç Uªk?…²Þæ01?€ç Uªk?ïüÂ¥Bá!?@u=à̀Ç?9êÕèöÿâ?@u=à̀Ê3FGL J1648.0+4230@PÄ:}ªOÊ@D÷œ"/¥À:kªKÀ;òÛé B*¿Ô\È/%©Õ@|s(@»Ý@×mŠNοàC±‰`¢"¿éæï'7ñ¿âŠ
î¥H¿ïç»ÊŠÁÿUNASNonenone?ïõ§è¿žž?aÄqQù"#?T°.€ÂÅw?aÄqQù"&?îÀVWu¦?§¿÷SzM«?£úšˆ¦%š?§¿÷SzM«?àÏ5?™"¥Ï¡ñ?¤·îqó¢?™"¥Ï¡ñ?ïJ5#Þ~P?z{V?–¹["05ý?z{V3FGL J1648.6-5635@t·k¤"ÈŸÀùõß덂À9CCÁð`À:ýàl¼Á½?ôSÈ)$@
)œ–¤Ô@hž\‹¿ãžõ"YŸ¿î‡Ú%—¿äJÅk¿ÐŠÙD¶UNASNonenone?äá)¢5ã¸?ÎÍÙËîY?Ö=¬»"8?ÎÍÙËîY?é5.Ãd??уõ€?Ë+Dòo§?уõ€?ç_fí¢@–?²te¹uÛC?ÑA2$»~Ö?²te¹uÛD?áKo=œ?Æ÷oi¶2Ì?ÝÓhß!"É?Æ÷oi¶2Ì3FGL J1649.6-3007@vð¹@"Šl~®[ÈÀ9
д¸ÙÑÀ;!Š{¥?òEaƒ¨–@¸¦Í^Ã@"É﷿ߟ-ý¿3¿äõ힇¿â˜µ˜þ"¿ïÿôo±œMUNASNonenone?ß1
-¤!?Ñ¢œÂêN?àgyi­ð?Ñ¢œÂêN?Ñi,ÿ\?Íd¸ÕhE?çKiñQþ?Íd¸ÕhE?є›å?µ÷­³Lœ?ç5ž¿p2
?µ÷­³Lœ?Ñ=çlä·?²t£¸¸t?ça}ɍ¥?²t£¸¸t3FGL J1650.0-4438c@uMIº^¿–ˆë¡y6ùÀ7P+ÃÓ)À:
™Îr¿:¿´ñ{Nr,W@Lóin¯@«"¬î‹¿åU5_™~Ó¿ç²¹'[ÿ¿å™»µÎ- ¿ë	—B¯0UNASNonenone$?àEœjy†!?ÐÌ*;;eÌ?ßtÇ+ó¾?ÐÌ*;;eÌ?Üw¦TçÇ?×[W²Ÿ?áÄ,Õô?×[W²Ÿ?ᮚ¦r?·ÊŸÿb°%?ܢʲÅÑ?·ÊŸÿb°$?ìU¡o‰ÆÝ?¹}Q‰?½Rôƒ±É?¹}Q‰3FGL J1650.0+0356@5Û;BÌ-k@<®ð®SeÀ:)CæÝõÀ;•ÙÔóü¿ÕøD¸0@[ÛB±Ux@S€?ÖY¾¿é¹€á¿â6 $š‹~¿Ý["¾¿ÖLn£UNASNonenone?ïÿÓŀôã>÷wåôrHà>ö?…Ž}R>÷wåôrH ?ïØœ!ëÅ?~"¥l¯ìp?sÀ1ï
}?~"¥l¯ìq?ïÞlž¶¤W?rç¡B¯Ç?pÉ°¤­Ô´?rç¡B¯Æü?ïý›þ ?4Y~w'{½?7ßû ÿ?4Y~w'{µ3FGL J1651.5-4626@u9²þÅm]¿ö~'MKãÀ8ÿÔqܼÀ:2¯È¿ÿÛÂMíɝ@
dy¤†²Œ?þ¿+ie?ç"LšÀÇ¿ãi‹™Ì<¿àŒŒ¾¿Ä¿ãì·£2UNASNonenone?鉒"‹rø?ÇzŽF¸æ8?ÉÙµ±Ò4?ÇzŽF¸æ8?îÀ¾ÿéAÚ?º"w
ôF?£ôkâb?º"w
ôF?è`Ý4º ?²Áp;@+ƒ?;|‹-}?²Áp;@+ƒ?ïþßT9?9š2>|ÒF?"
¶/Ld±?9š2>|Ò>3FGL J1652.2-4649@u5ö_Ø­¬¿ûàÛwŠ{À8¹°,À:=yaë­c?™g¾yNªÆ@ët±­·‰@»ÍŸ°‰ö¿êí\Ò
q¿æÝËu'[ë¿Ö‰óü3B¿ãክ~ºUNASNonenone?í6áôĞ'?º Êl/°?¶HðYÛñ?º Êl/°?í?"€?ÂÁäÅ£—ä?¶ÏYì?ÂÁäÅ£—ä?éØm˜y?´¾› ƒ­?ˈžIž?´¾› ƒ­?ï¹oDîÁ?ˆ"VSb
?¤9.ÄOµ?ˆ"VSb	3FGL J1654.0-4617@u?ž£Y5ü¿ùҌDF€îÀ8Ձ×ÛôˆÀ:a6=©®»?íÖ¯Ÿ?uâ@[ã‹U38@Ÿø-y?åÅ°óADˆ¿è6
g¾øp?Öñ\Û¿âSY<÷UNASNonenone?ì{2ªº†‡?¿;sJ'?¼&jª+ËÃ?¿;sJ'?é€r?Ñ(Yí2î`?Ëû©ÿŽ7ú?Ñ(Yí2î`?èð-v½Å?²äÞj Ôü?Ì?J%¼ð?²äÞj Ôü?îˆYòg Ë?­Ÿ)ð^0ê?§z`مóJ?­Ÿ)ð^0ê3FGL J1655.1-4644@u<`ÔV.ÀO¼ä!}(À9GeÆ-vÀ:jÏЍK­¿ö'kØ@
«Ñ?þäw¡!MX?ïýt&Ù?¼ú]‹˜ÇY¿ìDñ/
¿Í)ȃðnUNASNonenone?íW®Uóæ?ºã"qæ.¡?µBP`Ï?ºã"qæ.¡?ïq‡#?³Îãa?ŸqÏN[°?³Îãa?é"tûöQ?°TÚTxN?Ëv/¼&¼?°TÚTxN?ïüËÉ*h{?In¤Ç†m?9¡¶¬¼%Ñ?In¤Ç†i3FGL J1655.5-4748@u/€IQƒÀ1Ÿ<pɗÀ9	ñ}†=œÀ:v¦ ™@¿÷ú­¥ë§@'6µð@ü½¿h¶"¿äBVãVž¿ë}»Áãe¿çìѓ'¿Ñfn`¨-ÓUNASNonenone?í"Û¹|ÃM?³	èÜя?³Y"4åš?³	èÜѐ?ïº9j5"?³.—åYýµ?œˆ¸Ò¹M«?³.—åYýµ?èøV‡±p?³§€·­?̧™á:B?³§€·­?ïþ×vÔÁž?.AwæfŽ?"ˆ'³æ0O?.AwæfŽ3FGL J1655.7-4712@u7P›ùÆ*Àhñ[!ŽÆÀ8ìùTëàÀ:O7iù˜Þ?ã·Ñ$m@
ñk?¦@ൟ´Á?ïÿÂ8&ì¿êú(­Âý¿É
~XJ™×¿ècÃ`\UNASNonenone?ê—ø"/A?ÊL¯V$G?Å ïBû‡?ÊL¯V$F?ì,ÜW(7
?ƁžˆµP?¾™F¾Gµ?ƁžˆµP?æ¡uŸüÿ?´qÊ8`¹?Ò½ÀÛ?´qÊ8`¹?í|²¤s7Ë?¶pBíõòÜ?´jÜfA¨?¶pBíõòÝ3FGL J1656.9-3919c@u›ñ©ûçm@«€>~ÀÐÀ8ÙZo¸ÀÀ9o+-«3ö?îuƒ2Wž«@
pµÕduö@ŸÁàŠ™Ì¿ìzÛd%¨¿ä>lbm¢¿â~­®Ñ¿é¶Z'àùUNASNonenone)?³õÿÑÆe?º–ïñvç?í@Ç3]?º–ïñvç?êxgËԁ9?͚?ÑÚêé?Æ`Эû?͚?ÑÚêé?ÕÁ`=ÈŽ?¶/VÝ®Ü?åOáñ¸?¶/VÝ®Ü?äѾ"q?Έ[)[i/?×Ð\'Öå?Έ[)[i03FGL J1657.6-4653@u>tSŽóMÀÙï_žÌ	À9à>™˜ÃÀ:zBf¬ÝC?Ò©BeøyÆ@!ЂŽæ@i=@}H«¿íޛ›^?ïý°X瑎¿ã¯ÉÈ4¿à"‹Y"‰UNASNonenone?ïg@±•¤Ù?œrÿø,¾?"éÍKdî?œrÿø,¾?îæ©u¬?¼M-Ì´þ!?®¡Ÿåh¥3?¼M-Ì´þ!?ìÚ>õ¢?¬I0ó@'á?¿9/ŽRò?¬I0ó@'ã?î÷xŽÙL?¡üÖa×îÝ? ¨wk=?¡üÖa×îÝ3FGL J1659.0-0142@1¥Åo@7èSŸºEÀ9E¦N³Â:À;9ÏÆl`?ç2ˆ?¡x@$'RxGå@Ž™`cÂó¿Ùœ{©Í!¿ä𫲱ÿ¨¿Úþ£ûXŒš¿ëÃy¸sUNASNonenone?íB
Sd^?´ˆ'Q‰í(?µï—UdÝ?´ˆ'Q‰í(?îL:¼2R'?¨™É©íüü?«<T<Úݜ?¨™É©íüü?å‡úB]?2?¸×4ÕR
?Ôð{Eœ?¸×4ÕR
?êÍ\|L?¯T=‰?Çû˜ÊŽÑ?¯T=Š3FGL J1700.4-4019c@u•ê~ùÛ#?ó/ˆƒÇ À82NÛËÀ8—"€ãÀ?òw"pèu@Ò]×K«Ð@'¯ŸëBY¿áÔ.LæÚâ¿Ü|ùÁm¿ëå¥:%"Ž¿å&"g3HŠUNASNonenone$?'±/"ÈT?£Øoúhƒ.?ïwâv†é¼?£Øoúhƒ.?ç–Ñ1±0?ѪSþTi?ÐÒxݜ ?ѪSþTi?ÎZS"î?·{Ô#íïê?èi~kþÅ?·{Ô#íïê?å!uCdc?ÑÓž,?Õ½Ãy79?ÑÓž,3FGL J1701.1-4930@u# ¥&•–À42ðîÀ9peÓÀ:«Wãä?퇩Þúæ@'$«@'ÛŸx€Å?¿hf±9ôC¿ì+4>ԅ¿èóO™'¿ÌŒ–"w8UNASNonenone?âLÂWmÿ²?Í´À'\@?Ûf{Q$œ?Í´À'\@?í&,Š¡²?ÁÙR¿"s?¶Î›ªòo?ÁÙR¿"t?áó¤Cí^?½˜ò€Z¥?Ü·x%CÓ?½˜ò€Z¤?ëšîÎ/í?·tBµßÊ?Á"DÇ@L?·tBµßÊ3FGL J1701.3-5216@ublvKÀüÂ]ÞÀ9‹i"ÙHÜÀ:öÔ2ò›"¿æzB÷ÔëÞ@4Èaƒ(@Ó«@`m¿á|_)¹À¿é|Ρ}¢¿ë—¨ÁæÐë¿Ïß:sCoUNASNonenone?ï6ï3‹>
?£yÂkã5?™"Ž˜>¿?£yÂkã5?ïMêQ¿«J?¦*¨Å`?–BµÈ
–×?¦*¨Å_?êd•~y(?¸;ô?䢃?Æo±ªa?¸;ô?䢂?ïç€s" í?gðÍ29Õ?hŒk_Ë?gðÍ29Ó3FGL J1701.4-4654@uD¶°_¯À÷d»k{yÀ8M·Ñ"+À9ò™°?ÎL?ñˎ6.í@Žà®.@àyQû¿ßwB(æË¿ê¾þ¬Ý‡õ¿æ¢	sWvÆ¿ì¯2ՀiUNASNonenone?'öÁV­"?š/[ÅW•å?ïpIõJ—t?š/[ÅW•å?ÞøW!ÿP?Õ,¿ž&.?àƒÔ?oX?Õ,¿ž&.?É©ìº0ߊ?µ¯áËu?镄ÑsÈ?µ¯áËu?ÒĚ³:?À€hXá;?杲¦bóþ?À€hXá;3FGL J1702.0-5414@tçõ£KÜÀ"VÿÁßÀ9°—  À;-X'ßB?í,ýÜÂÂ@𽢍^@ càz(»¿Û}ƣפܿéʓõÉMð¿ë]b¢E¿æÑÑ䎵eUNASNonenone?ëƒpoÑ3?ÀÔѨ{yf?Áò>CŒ»5?ÀÔѨ{yg?æÀ@¥©ûÑ?ÒÊIóDk?Ò~´¬^?ÒÊIóDk?æ.š×¸•š?¹¯‰ d}?Ó¢ÊPŽÔÎ?¹¯‰ d}?ào[Sš¹?¼Ð¨ÕC*‰?ß!IXʍ?¼Ð¨ÕC*‰3FGL J1702.1-2524@vWñ6;%@#÷Úè'®À:>4ð¢"ëÀ;_$Ÿòy/À
tq£~@	ºˆ\Zsê?ü&C@qŠ1¿ï§Í:Ÿ§ê?äiáp¦cà¿æaW1rÇ?ÈÕ%‹Õ·UNASNonenone?ï륳w?c¸–|™
Œ?déZ€L‰?c¸–|™
?ïâcd
ýp?~Êbö¼?mœ›òd?~Êbö¼?îÙ_^݃?"ÌÿÅÕtk?¢j
'Ó?"ÌÿÅÕtk?ïÿúw0	·>Üe¿…ôý>Æ#?Ù">Üe¿…ó˜3FGL J1702.1-4623@uLw[0À,Ò@ª;À8™Éõ÷¼À: 2:ð?ÑOš+(¼|@Xî>Œ'°@Cà) ã¿êÀ`*76"¿çèáçwY¿éG»¼•XS¿éÀNº«À–UNASNonenone?ז"¦î¢3?ÏÀ1G?¢?ä4¶,ˆ®ç?ÏÀ1G?¡?íld(=""?¿qsLòÕ?´œÞ¾[e?¿qsLòÕ?áÝÜp—yP?µÚ
»«?ÜDGÑ
_?µÚ
»¬?í]<2²ü?³À-SQ?µÎjh#?³À-SQ
3FGL J1703.6-2850@v.¿œb¡¶@™?¯BxKÀ9Úæùž¼ïÀ;1ç£è§õ?ÔîÒ¦U"²@
T£ºM@ЕÀœï¿è¬RV9¬¿ß‹^žµ§¿Ýhm¼	õ¼¿è1[âÔËõUNASNonenone?n=x´?"§¶€·?‹äp¡Òú?"§¶€·?éJìî}y?Í×Ú¯*¿›?ÊÔLF	Â?Í×Ú¯*¿›?îi¢Á«\?¡b"‰r{?®ÉeÓåJ3?¡b"‰r{?âÇÕù¯_+?ÂgÔ ?ÚpT¡Aª?ÂgÔ 3FGL J1703.9-4843@u1³:}ªÀ¾ «†+À8ÀUM9n·À:¦ƒɕá?ôƒŒçÚoM@
ÉfÅ=@àVŸsù!¿æð¼ÍóŠÉ¿á€Knµ·ª¿ëMkÙ xd¿ïðÊã
]UNASNonenone?VL‹ØU}?`ãPôÝ
?ïôÙó:Õ?`ãPôÝ
?šéD§ú¶?µÌžå³?ï(µÚÀ*O?µÌžå³?·urÄe,î?¦xAÏó¹?íQ§sZb?¦xAÏó¹?¦±3KfÕ?–›'Gäu?î—ìËI'?–›'Gäu3FGL J1704.1+1234@@;‡½Ï@=l§qÉpøÀ9d¼¯HWˆÀ;|ƒ-±¿ç¬LT'£@Í,݃©B@ªŠÿwïÑ¿çÌBºÔk–¿è᫦·d[¿ã5àçX`·¿âùs–G!UNASNonenone?ïüú'[î¦?A, '?8+u ŠËÖ?A, '$?ï¾Aþâµ?‡±©gû	?€o€GR¼3?‡±©gû
?ïk›±º˜W?ZVyU÷_?'Œ‰È¬õ#?ZVyU÷`?ïã>íI­?fo÷¬/4~?lÁ¶Rr??fo÷¬/4}3FGL J1704.4-0528@-Óp&É@4̽±¦×À9Q!Ð4`ZÀ;1°(QWá¿ðG˜7™ÊA@
ÖHtÄù@zZ Šy–¿·pCR…Ëì¿êW1zKuŸ¿ËdöU¼¿åù…µê¶UNASNonenone?ïëhòá?h
'¡ãæ?d—ñé
?h
'¡ãç?ïÓsmã†?€'gGȼ?vFuÉ<ð?€'gGȼ?îi9"Äky?žGøJUüÚ?©lf³¹Ho?žGøJUüÛ?ïó?0Ä?`ñ¸cšéÚ?Y€ážwüö?`ñ¸cšéÛ3FGL J1705.5+0948@=ÃRü&V¬@;ó~€8Ÿ"À9¤œ«fKÀ;v¬Ö(–?⠝^då@žæ$a´@sï< ¿äËߏG0@¿ëº'fZ¹¿éØ/_Ìî¿ïþ±Ü[‹UNASNonenone?ï™,`'w?Š˜&¥""?‰´çÛ¾"^?Š˜&¥" ?èè ížÀo?ŀà¥ÌüK?Ì_|I"þD?ŀà¥ÌüK?íÖä5~P)? "Äc²ln?±HÞT
~µ? "Äc²ln?ÛìÖÈcÏ?·¬zªã/ß?â	"›Î~™?·¬zªã/Þ3FGL J1705.5-4128c@uÕϪ͟¿Ñük`v7jÀ8A[ñ˜^0À9?m?ﲕ:õ@{õ¬"óí@#9ßÊ«_¿çrèf›‰¿êãýVb¿àÙ¯Ü|S¿çÖ·p³áUNASNonenone)?ÕxÞÕ£—ä?Î{›(°?åC•.4
?Î{›(°?à":ñù?֐éaÝ?ÞًÚ
?֐éaÝ?Üt—+¹?·¿iR?áŹu´j#?·¿iR?æó'‡Ï?ο…E'Äè?Ò°ñÑÒc?ο…E'Äè3FGL J1707.8+5626@U-þ®û+@B@­ÿ'+¿À:THùn‡À<«ƒ¦é
?ÐA(J29t@
±[UçH@
¨_°Ù¿íÞ¸1+¾l¿Ô}À³l‡¿åY
^¨Ä¿êJØ3ÙµUNASNonenone?ë L²¼åx?ńÿÊZ¡Ã?Ã~Í5j ?ńÿÊZ¡Ä?ã
uŠÅ9?ÒWÞ^":?Ùåêuò?ÒWÞ^":?ë&1±c?°""^L?Ãg9;ÂsÒ?°""^M?Ú2½!?Ã]º?ÖÞq?âæør!o?Ã]º?ÖÞr3FGL J1709.4-0917@(d ]Øù+@1¹‹Å›€$À9ZtŠìW­À;"Øzøß?òŸDFx@L'Ûç@·Ðß´0¿à°2x*è¿ää0ÌÚj¿ï¡a+5…??ÜH¿,âGoUNASNonenone?êðv[?Å.Û{²†ã?Ä>'þ"¹þ?Å.Û{²†ã?ïSŒc|í?±‡Ë¢¾€?•Žs}"u?±‡Ë¢¾€?æŠ^À‹š?³""xœs?ÒëBÞèÌ?³""xœs?ê'èI.`?Å2M¢ÖD ?Ÿ_¶ÛF~?Å2M¢ÖD 3FGL J1709.5-0335@1Uœàuöý@4²‰üm¤HÀ9\åüH»[À;*½é§Ï¿Ùijû@&ë$üŽ±@Âb€}¾È¿ç;£g ¿éT_0o½¿à§mƒÕÑÈ¿ïýåғqsUNASNonenone?ïéèƋÐw?qóҜï8?f9t/ˆÍ?qóҜï8?ï\µ/ ƒ?˜›ïVÐl"?"iZïœÈ?˜›ïVÐl"?í+:Áð?§Hì´í3?·Î¦/!ð}?§Hì´í2?ï:'"~¢?"÷*±̼?˜¯»°+¿8?"÷*±̼3FGL J1709.9+4624@R÷´·@B1C¿rq7À:\ìOIoÀ;ðö'9)í¿ñ>ÜÔ׳0@
öÑÁŸ}@í ,ì¿äì>
ì[ø¿éÊñ"žÞ¿ÜI˜Ol¤Ä¿èA»püUNASNonenone?ïÿ\˸?-žÈ?Ù"?fˆýEq?-žÈ?Øþ?ï¢àö±:?'ŸN_Aÿ?‡GÂS±\˜?'ŸN_Aÿ?ïqÖ;¨®?Œw¡bÄ&c?'Å<8ŠêN?Œw¡bÄ&c?ïñúIj?]ò×–¨?]Æmï+)?]ò×–¨3FGL J1710.6-4317@u'•éᰊÀãâ;ëiÀ8£bþÒÙVÀ:3T9¿ç+"Ÿ¸I@i›Â"¸Ú@6¤€}há?ïÞIρÝæ¿ê×{»Ñ싿奡mV"¿ç"§4•fUNASNonenone?ë:p٘16?Æ1/+Tqã?Ã<™Ÿ;(?Æ1/+Tqã?îÂÞaczg?´"Ð0øBó?£ÒéÈYˆ?´"Ð0øBò?åFl™ˆ"…?µû"þñ} ?Õs&ÌîÖö?µû"þñ} ?ïÙ£;…»"?|sË´"p"?s.b="5¸?|sË´"p"3FGL J1714.6-3327@v	9-Œ*@Q]À¥wÀ8ãÀÏhˆ€À:u¡¥×•~?èXç³ê@Ú_c<æ:@ۙ wï¦?ïû7»'U¿é¤f"a¿Î'èÉ
S¿íyü‰ÐyUNASNonenone?ç)óe8rÙ?ÎÌ-óa£Ñ?Ѭ5M?ÎÌ-óa£Ò?ììurÉ""?ÄÚ[úoǹ?¸œTi¶ëh?ÄÚ[úoǹ?á¨Ìêvó?·Ì*hd­?ܯÜf+?·Ì*hd¬?ì^牮á?ºÞYpD@C?½Hòˆö?ºÞYpD@B3FGL J1715.4-4028@u¯vݬîá¿òÇAÝðáÀ8çw ÈÍdÀ:qΣf¡ö?Ô©{¨±©@^9ókÇú@ÕYŸ®†'¿ïٙ{‰Ã?äæBÙ泿¯ƒû¿û¿á°ŽJ'ÛUNASNonenone?ïÎٓîÆ?'è
­Ñk?xô6I?'è
­Ñk?ê×8ãz%Å?ÎGІˆ?Ä£rhì?ÎGІˆ?íta•xUw?¦ý8ÙÒ:p?´\óT=TF?¦ý8ÙÒ:q?ï½ÇŠƒ£?Ž-ÒKp–?€Ž:_)?Ž-ÒKp–3FGL J1717.6-4404@u"^Ñ·ÀÌ2ùQÀ8nzj)i†À:n½º
Ri?ájÜÄÞä@›N•dUÀ@s¿ÀIÝ¿å \ÂVYÜ¿èl¬yxÅl¿ëºˆ×çC¿ãšá?S0UNASNonenone?㽿êú2Z?Î	ç3Tªb?؄€*›L?Î	ç3Tªb?èUœ¢Ì›=?Љ}*ª?ٍt͓?Љ}*ª?áœja	ܚ?ÀâÿùØK?ÜÇ+=ìFÌ?ÀâÿùØK?çµîîoþ?»>v¾1ì?Д"#õ ?»>v¾1ì3FGL J1719.2-2433?ß&•á(N~@E#ŸAyGÀ9Øïþ¯À:ëьO.;¿ê{—Ùƒ@
ti?´¡@QÓøÿ¿é®z'/Î,¿ëlîïr¥J¿Ó‰Û
àÆÝ¿éu;ss•#UNASNonenone	?ïÙÃh¡K‹?y¿hdBH?sK¯Z:ê?y¿hdBH
?ï¯Ècÿ^?"Vþ1Žb\?"
û'(‰?"Vþ1Žb[?ì'FþìœQ?¨»–ng«?»uÈ›x?¨»–ng«?ïàQޒ2?rÀYV¸£?o®!mÍõ?rÀYV¸¤3FGL J1720.3-0428@1þ}ÔA5@1ìaAcwŸÀ9àÎÏÜKÆÀ;1s?'½À6·$ÄÛ@á=1¹¶p@°§ÀMãc¿åq3†6²¼¿ëØq›Dœ¿ÝèL@[ ÷¿Ï0Ÿ\H¢©UNASNonenone?ïÿ}aÔÛ×?•Kaßå?SÅd…^?•KaßÞ?ïä¡:Œ>¤?w6WŽ˜æ\?k^ÅsÁ\"?w6WŽ˜æ\?ï's,ßZ?ïŠ'g¦?‹£4È)~?ïŠ'g¦?ïÿþ<à^Ð>À¨\:Åó‹>¬1úúC>À¨\:Åù†3FGL J1720.7+0711@<ÿAJM+,@7i㸡œÀ96BhZ\mÀ;MbXº¬9?Þ9ëÜåý(@IŽ"«@Ï€oÑõ¿ãý>QŽ,¿ãgnöÐ"å¿æV	–¤=¿çãr3WŠUNASNonenone?åóøjP­?Ëx|]Ñë?Ô+ç^¦?Ëx|]Ñë?ë"¼"Ë©?ÃQCD€¾$?ɱtÑZ?ÃQCD€¾$?éiäZ…Á?´I'ððI}?ÊXoº•èþ?´I'ððI}?Ⅱöڇ?ºBÊïvCé?Úô½Jò?ºBÊïvCé3FGL J1721.4-5253@u·AJM+À"4!ž¶9
À9Dð(§üÀ;@Ø7d¿ÎÓ鿪X@
&<(zGš@­¿cØ¿ëÈÌ@ϗǿÞdÖB[3¿éó]†T(²¿éêF~OÍYUNASNonenone?ØS(×|ßé?Íke¦üFa?ãÖk"A?Íke¦üF`?è]bù3©á?Ð"Jaøì?Ίt1Xz?Ð"Jaøì?æ_eº\?³‰ëÌ2w?ÓÕA4‹ÁI?³‰ëÌ2w?ëÜ/?£à`?²Søڋø?ÀCp~}?²Søڋø3FGL J1721.8-3919@uÉÑc4'¿¿øs
=³À8·5@L À:B·
èa¿þŸ>+´¹±@A
•iß@Xwœ'"¿í±6i|#¿ÒSüÖC²Ì¿áã6+h¿íbZidz¢UNASNonenone?ɐä›yQ³?ÈzŠ²í¡Í?é›ÆÙ!«"?ÈzŠ²í¡Í?îˆ:ޓ¤?¼ýëÅÜÝë?§¬RÅÄ?¼ýëÅÜÝë?à?Úzçv{?´Å#'‹?߀K
1
?´Å#'‹?ï÷Ñ[ï?i$Ás'Ž?QÚ]H!è?i$Ás'‰3FGL J1722.7-0415@2~µ^ñýß@1"BÇû¬´À9‡YûôÙÀ:æ+Íä$?ôëG©·ÉÛ@7´»³õ»@[ü€¿?ïûǪ+À¬¿àñ†»»¿ènÂ+øÆ¿ïÿ›ÞIàUNASNonenone?´T0à>å?Â1]1–a_?íuyýCø$?Â1]1–a_?Ÿ®õ"'ih?±Æ!¼Ãq²?ïˆSfÄ´?±Æ!¼Ãq²?¶‹ßʽä?¥xªì‡?í.œ"¨D?¥xªì‡?Î8ZFÑ?ÅCǙp?ïŽ=/%Ê?ÅCǙp3FGL J1723.6-3646@uîΤ¨ÁU¿Øsš×\HÀ8›EÏíé}À9¢P¢¯ÂÑ?æ%c¤·@
Áñ§w¨®@Ìh€Z?žŒä¹ÚU¿è,E·3!¿ä*ï-†P¿Û£±[¾RóUNASNonenone?ÁíkE"ç?Ǟ
çO´?넥.ŸšÇ?Ǟ
çOµ?ã—¢Üñ,?Õß,†èj/?ØÑüºF¦?Õß,†èj/?ۈ¦™Õ?¾JŒy}ð?â;¬À38?¾JŒy}ð?ë¯Ìh_w?Á'^™!6?Á@ς^'%?Á'^™!63FGL J1725.0-0513@1ìh¹ý½0@0&cAøÀ9´â:¸cÀ;ÙÁfg¿ô¸Î¾¡@Û\ÁL$@%ÄÀcÝ˿ǃõ…0"¿é1̋‰`'¿àz»÷¬8¿Îxí|›UNASNonenone?ïû…	"á?Bqû+×´?AëÙËt{Ã?Bqû+×°?ïàá"2€\?yœ$,L'?olÍ£‰?yœ$,Lƒ?ïM©¡"¥?³'/'gD?–JËݛ«h?³'/'gD?ïýîßA(þ?5u4è玶?0‰ö¸"?5u4è玧3FGL J1725.7-3555c@uý—ÿCB¿ÏBwß4®]À8+Þº5"À9O·Xâ?Ýd"¼Ð@dZ­ Œ¨@Àè€1"¡¿ì·ºýþ";¿ãP¨¸V¯J¿ß‰DL`*ã¿ëw­þwâUNASNonenone0?ÁÂÍy¢º?Ã|™Ë×?ëL¡—?Ã|™Ë×?ã'
«]cï?Ö>+²Bê?ØÝä©E8"?Ö>+²Bê?ßÇcõzC?µS°"?à~NBÞ?µS°"?ìJß8"?ÅDüôË`?¿gí©;q?ÅDüôË`3FGL J1726.6-3530c@vÑ·Xâ¿Æ'ÍúI\ÀÀ7£-0º²ïÀ9‹Àނ÷?òÄïc$½z@eÛ­m0@u¹_݋6?ìဌò/¿æÐZ\± ¿æRT­p)ø¿ê΍Ÿ:mdUNASNonenone$?ŸÆ(Béê??¬^7"!9´?ïν谮?¬^7"!9´?ÏÕ!Êû²?Ñ+Ú3š?è
·¹
A?Ñ+Ú3š?¾ó!-ª?²?Àwô?ì!›Ýº\ª?²?Àwó?Ú©U Š(Ø?LJG©w¤®?â«Uoºë"?LJG©w¤®3FGL J1727.4+0634@=6cÇOµ@5¥yžQ?À9‰/Þê܂À;:³In?ï.ú81¤@W]"Dù@&À36c¿èEw¿çx¡È£X›¿êÝ\îSÁY¿ïùAû«UNASNonenone?çñËòËEœ?ĤfÝ}Û'?ÐhitÉ?ĤfÝ}Û'?àœ½ÉöB?ÑW\"zÛ?ÞÇڄl}?ÑW\"zÛ?èW´åüðž?²´np¾<?Ρ,h=ˆ?²´np¾<?Á	>2Óö?¦¥$ËÛc.?ë½°sz?¦¥$ËÛc.3FGL J1727.6-0654@0Á‰&"Ï@.AðÃLÀ9A 6×,¢À;>Ä`î?âÎqê iº@H³SÜK@¬M@O¦[¿âC<}‰ÃŽ¿èó|Š¿äw‹pû¯}¿ïÿ݃±Ù_UNASNonenone?î+³}Ý5?·–à(Ú¦ ?­DΨ",¬?·–à(Ú¦ ?ër'?¼ç?À>ìý?Â7cðf?À>ìý?è[[·òõÃ?µùøO<œ?Β' 4(ö?µùøO<?â¥?Â6Ó?»¼!*WãÕ?Úµ€{'[?»¼!*WãÔ3FGL J1728.0-6446@tvÌcñA À0MÛU%ÌÀ:¾[
À;¤®ç¸5?™"¤¹É"þ@YKÞzÊ!@Nº€D¿ê$­´Y¿ç8Q¥¿íÀ¢ox€¿ïýb¼¶UNASNonenone?ïë@«òÉ?j²¼'ŒÊ?d¿Tþ
7 ?j²¼'ŒÉ?ìÈ(™"Çð?ÅPX^¡Ö#?¹¾»3aÀ'?ÅPX^¡Ö#?îÙGéf?•§Aõ	€??¢kŽ¯i?•§Aõ	€=?ì®
.'(?©pt…3U?ºŸ®‹n¼?©pt…3U3FGL J1729.0+6049@Vr¦óõ/Â@@µ‡?úÁÓÀ:WQ§'€¡À;¢µ'ôcë¿ëMT¶T"@ÒU ˜ÑÉ@-ž_§'¿è`
rô5¿á/èSÍÜ¿ìDƒŸÝ+¿áôÉʨŸ
UNASNonenone?ï³/òØ$H?ŠF­¦/?ƒ4Iöíô?ŠF­¦/?ï@÷um*A?§°Õ×?—áRZ·ü?§°Õ×?î ÎÅ]S?Ÿ!‰ó#Í8?­óª/êÐ?Ÿ!‰ó#Í9?ï‡EE–ü?Š$— 6n?Ž8®®šA?Š$— 6n3FGL J1731.9+5428@TŒ]á\¦Ê@@"ð^¢LÇÀ9Ò®Q·'¹À;Ù
£ÇðÅ?ÜÑ-<¬·6@
_hT'I›@7#_ÖS¿çފƒu•¿ë€"È×Ë¿ëÄ@Hq-¿ïþó…?¼ÑUNASNonenone?ﮅòuÇ?†ž÷%á–?"^ºbŽV?†ž÷%á–?á›éà6¼?Ðwš-Íá?ÜÈ,?ù'‡?Ðwš-Íá?íëyYŠ^? oV°ÿa?°§$53­? oV°ÿa?Ö¼ZÑÑ?¾	¤˺?ä¡Ò—sx?¾	¤˺3FGL J1732.4-2709@v×Ûôˆ@8™aeu¦À8º­²URBÀ:Wè+Íä$¿þëÖj…Yò@"v¸@ûԀ Nj?̧¸ÃL賿ê•`;¿Ýû–EɅ<¿ç"´ìA˜bUNASNonenone?îÇË£?±"nÖz?£ƒNEÏø?±"nÖz?ï±
Kê<²?¦rÔ/cZ¸?ƒ¼­pÓ\?¦rÔ/cZ¸?éä<ÅÝA?°ê@QF9Ö?ÈoèŠûÌ?°ê@QF9×?ïÿ5z?1;"æïç?™P¼®J¢?1;"æïçi3FGL J1732.7+5914@Uøo?Rü&@@ƒô#Rë_À:úkáÐÀ<®âô?¨«CLš@)¿A@S f'?ïŽß{r‰'¿å?Ç7%tó¿ä{þi/¢
¿ÅQwnUNASNonenone?ïõ{ë–ìÅ?^ MLÿÜ@?U(Ò&v¥?^ MLÿÜA?ï´áªvÞ/?ÍxÝéf?'Ç•bHt?ÍxÝéf?îédY´H5?–Ï*! š?¡iºd»|¯?–Ï*! š?ï…7ãÓÙr?‡©·µp^>?Ž²	£­?‡©·µp^>3FGL J1733.5-2811@vsw[0@#lfZ§ìÀ8Ã=dRÀ:.¾ÐŠÇo¿äРÅœ´@b£S&@é¿¡Á¿ÀŠ»î‹Áó¿ëòƒ
¿åàèϦŠ³¿ã—KOx}UNASNonenone?âC| Ü·?Ðð¾û"ü?ÛyɾF?Ðð¾û"ü?ïŽÿŸŽ0q?¤d<ø?Œ@sãð?¤d<ø?åǐQø?µg;àO?ÕöqÄß\?µg;àO?ïÓOå®÷=?}Žn‰ð?vX
("`ï?}Žn‰ð3FGL J1733.5-3941@uØۋ¬q
Àâ1ƒ/ÊÉÀ9&/ŒEÀ:É+üLû?ÞC+9zÜ%@­OoÔÏ%@×àŽ¾¿âr¶ì€Ø¿ê'WMKt¿Ø'å¾òTؿݨ`'CLUNASNonenone?ï¤ÀŠœ?‹··"úü?†Ïø[Øô?‹··"úý?î¢êsȓÓ?´6ã4W`#?¥ÑXÃvÂÕ?´6ã4W`#?ìõ~è÷ì?ªàD/Tx?¸T¸Gð¬?ªàD/Ty?ï%I!I¦?¥~Öñ^Ú?›VÛÖÐX?¥~Öñ^Ú3FGL J1733.8-6056@t³‰ßrïÀ-‹:%•»¿À9poz^ÙÀ;'2{}NàÀX×æÜBŒ@%€˜Á­_@§©Ÿ¡—¿çN"kô¿æ-ø°R¿ì"ùTs¿¶G€‡UNASNonenone?ïáîâ¼?ð?rµN$
z?nCÀÑ?rµN$
z?ïÙø;#ÔÆ?1n™%ZŽ?sân1?1n™%Z?îðh*§J¡?–œ–'Îi? ù}U‹Uô?–œ–'Îi?ïÿïçr>êˆo58Û#>àñëB>êˆo58ÝÒ3FGL J1739.9-3124c@vT&Á½¥¿Ð†êÕÌOÏÀ8\+xSδÀ9ò5ýé?õ€@tº<&@zž¬¨ë@P¿ "_ž¿Ü`7˜r¨¿åӃZho¿çd'²ÕŒ¿èߪ4ùyUNASNonenone<?q½[R¡²O?w!$yC't?ï܅IZ¼œ?w!$yC't?ºëšÇŽj?ÀGß#¨¬ã?좌§.3?ÀGß#¨¬ã?¾Q»`U?W?°/<àú?ì5ȓõX?°/<àú?Ê/NˆùRH?¹Ù!Ç° ?ét,]Á«o?¹Ù!Ç°3FGL J1740.8-1933@º¡<ü	Ñ@NkawêÀ9‡¸·lxÀ:ÚwNëö^¿ý133‰o@5M6¿"»@²¾_v³¿àaKw«:ß¿ç<A³¥£¿áv…¥ñ¿޽çIÙEŠUNASNonenone?ïïtŸ`.?h¡žAÚ	?`‹`ŸÑê5?h¡žAÚ?ïÏÒxO_?Á(¼Ûã?xÃØvPL?Á(¼Ûã?íâÊ!ug«?¦¨¶²ŸóÇ?°é®ôT¨?¦¨¶²ŸóÇ?ïÿª\¥à3?6ªn¯?hևó
\?6ªnÊ3FGL J1740.8-6755@tRg ù	lÀ2¼8…	ÀÀ:Fšï/À;»\´5ýÀy
‰ò@`›csAì@O蠒Ý¿ça¶u¿èÇÖñhãn¿á'Ú~U	¿æ)wT—©LUNASNonenone?ïýBŽBò…?q[º—Y|?5ëèkÎ+?q[º—Y}?ïÚt'©²á?€Ž¨'6È?rž«&d?€Ž¨'6Ç?ïÊ#9êc|?wê±ò:Q÷?zîc
ÎB
?wê±ò:Qò?ïÿÕikè‰?ܾ¯(ì>õKJ»–.?ܾ¯(Ü3FGL J1741.4+0938@@âñ©ûçm@3ãý?[_¢À9vèõø?AÀ;1ÿD]Å?íº^?rÓÿ@À9Iøœ‰@ø8`nª®¿ß؎Éöj¿ë¤g¥£	§¿èpp3 …¿ïñ'½pI¥UNASNonenone?åfBC–æ?Ç}1
cª?Õ3{xÓÚ3?Ç}1
cª?åߐ®±Dœ?ÍTnô%‹?Ô@Þ¢vÊ?ÍTnô%‹?æ¢èhDá?´¹™å»I?Òº//wæ>?´¹™å»H?Ëùd•£?°ì@<¥m<?é¦Ú˜—??°ì@<¥m<3FGL J1742.4-7237@tgßã*À4à´Ê!!À9ùÖÌ*žÀ;¸ßR,¿ÞÞxžÕÌ@ 3&H@aÌà,¿ìé܉ûŽN¿èú¬Èº2¿â2úûM,¿å»¢ÆBUNASNonenone?ïýQ—w?77ㄈG?3õsDGð"?77ㄈ[?ﲘÌÍ`Œ?—íZ…I?ƒYÌ̧Üÿ?—íZ…I?ï'Ï·f?†ž½Œ|T?‹L8Ò9æ?†ž½Œ|S?ïÙ%=¥h–?h®7# Â-?sma-Kµs?h®7# Â(3FGL J1743.9-1310@*«ø˜,²@ õµØ",À9†·5ŒÀ;
3­¬v?ñ5£Ãi Ö@ó»Æû}@ærÀ'Ö¿çpïñü¿¬ÍÆU;%¿äv–9½»ã¿í¬ŸâKgUNASNonenone?Ÿ­Î<0V?©À5q\0˜?ï'Ž%?©À5q\0˜?á©õB	â%?ÐÎi}
 ?ܬ{ì;¶?ÐÎi}
 ?Ä"–úÁن?³6"ò¬r?ê÷ZAO‰ž?³6"ò¬r?ÕN÷`œ
ø?¶ÔŽùLü?åX"O±ù?¶ÔŽùLü3FGL J1744.5-2506@	0"¿íÁ9@¤±«VçÀ8&ÆÌ˲À:)}uv¤¢?Údúr™Çß@
Ó:ÉT;@‡À(N©¿æšø2šö«¿êñísˆ¿ã÷[ Üü<¿îart`UNASNonenone?Ø/h¯¶ß¸?Ðß<ýú?ãèK¨$$?Ðß<ýú?Ô/QI
ä9?Ò\{úƖd?åèW[y
ã?Ò\{úƖd?ááTAÇ8Å?¶"j¡'?Ü=W|qŽv?¶"j¡'?Ýnü\£??Äâ©1°i'?á~HÑ®`?Äâ©1°i'3FGL J1744.7-3043@vfÃóà7¿ès ôlNÀ7þ+i:V=À9Æú¤vln?î&U)s@F¬RÐÝ@æ›_Â]]¿Þúê—c	¿éðŠtÁ%­¿äÞ—fñ¿èÕ¨5
EKUNASNonenone?Ä¢æY&'?ÇíëŠ.?ê×Fi¼6v?ÇíëŠ/?ÙJ!âF?ÓÉÇû°'?ãZïÜü¸?ÓÉÇû°'?Ô~k¥c›?¼þá8ôÇ?åÀðÊ-N3?¼þá8ôÇ?äæe$­¼?ƞ"§Òi_?Ö35¶¤‡Ð?ƞ"§Òi_3FGL J1744.8-1557@&™»'ˆÛ@€ô"'òÜÀ9Rìzçý«À:î__áçç?å+Y Çd@ö–²‰›@z‡`%¿©ê7'õƒ¿äõþš'Ö<¿åjc㡜ë¿î–"	u°ÂUNASNonenone?¿è–•óé?ÄÆ<>)%l?ìí-\Áƒ?ÄÆ<>)%l?Øài›3?Ѷ²ä?ã÷Ë2qf?Ѷ²ä?ÛuÌ×u'ß?¹ììÄp¥{?âE"E>?¹ììÄp¥{?ÎÓîNcά?³ËCcӇ?èKlgV?³ËCcӇ3FGL J1745.4+4721@R'±F^‰"@>n9`sÞÀ:'ó²ê£À;Í
ÌÜ­À÷l–\ò@ªõ «†¬@wàyQû¿å`üŒ&¿éª¾UÌÌ]¿èHˆ&w'¿¨'‹‹ïøUNASNonenone?ïÿi+˜?Ó¥r¯áh?%µÚ!2?Ó¥r¯áp?ïݹ)"•?}ŠOЃ¥>?q#k65q?}ŠOЃ¥@?ïÕÐî³?t96¾¢?uˆò&@î?t96¾¢?ïÿÿí«É>wE¬#tn!>béT6ðî:>wE¬#tú3FGL J1746.6+0433@="¿¤Æ†@0}­ÙÂ~•À9œ-~¾LÀ;*þ±KÀúð¦ñ›ä@
{«lù¨@Ys_ÉZ¿åÇ\R׿ê¨Üäá°M¿ÚÖ\j[Šã¿é–è4l×UNASNonenone?ïõÇå'ä?ZÒáúÍd?Tp4Üx·7?ZÒáúÍ^?ïá/lZC¶?ypuRÐ@?nГ¥¼IR?ypuRÐA?î—T®§y?šy'¹«`È?¦Šµˆe?šy'¹«`È?ïÿD®úý±?(·])[æ?j  IÛË?(·])[­3FGL J1747.0-3506@v.cÇOµÀ§|{{¡aÀ8MRÓâjÄÀ:²	Bžá?ãšÛ—&3@ª½ÐZ¡@UÝw"q¿æ}"®î¿éÀ¬cÜÚr¿æa¶DU¿êaé©sΦUNASNonenone?íüï4Än?µihQU
?°†Y܋'?µihQU
?åŸ:›¡K)?Ò‰3ÌÄ?ÔÁŠÈ½i°?Ò‰3ÌÄ?æXˆ0h
V?·˜«¶F?ÓNïŸ/ëU?·˜«¶F?æ*~s¾/?µþÐý:k?Ó«Ûƒ¢?µþÐý:k3FGL J1747.3+0324@<›0aǛ5@/—Õ#³coÀ9iRÍ,nÀ;âµl]÷?¿€3¨4MK@
ã¤)Àn@Õ€ÙY¿æj2X¿âZÍÖâû¿áb¾Mz~™¿îWÂ?'K©UNASNonenone?Ó#`€ðÏ?Ë~Cô<?ænOò?‡™?Ë~Cô<?ì!ƒÒ²è?¿UaÇÌ´–?¾óájh¿)?¿UaÇÌ´—?áïh—aÌ?¿h–K¨?Ü!.Ñ<gÅ?¿h–K¨?èÅÒîø?¼¸~	"a?Ìè´D«¯?¼¸~	"a3FGL J1747.7-2904?À&'j(¿ÞZº LѕÀ72_½‹çÀ8í¸_~?ò«Ð}ÜO@·ýÊñ€`@ ?Ðû[¿â'†Là®V¿åÐ܎¶¼•¿æƒú¢Ý÷¿ê¬;ۀøAUNASNonenoneP?¹Íþ}ÿÎj?»Êç|jŒ_?ìÆ@0@3?»Êç|jŒ_?ØÓóUðæ¸?ӗpH°í?ã–UŒ¤?ӗpH°í?Ñïŕ'Ð-?·Åù[È"?ç5>—é?·Åù[È"?à9BJRÍ?Í0P?X½g?ߍ{kZd?Í0P?X½g3FGL J1748.0+2701@IêÊÿm3	@9\gßã*À:H—hfñ§À;ˀ
|ZÄ¿ô=$*ך@
֛	Ü!Ô@8Š`¿Z¿åùzíSwn¿àC8P Îº¿é¹">o¿Á¾ºì¶³AUNASNonenone?ïo8ù
9?–FD‹7?'ØàÞX°?–FD‹6?ïÛ:b±?|±Áׁw¨?rbòýN§'?|±Áׁw§?î!Ëo	É?¢ð¦'뢅?®
ãIc"?¢ð¦'뢆?ïý>¨H?6ó¼†Luy?6z¿m¿Ã?6ó¼†Luc3FGL J1748.5-3912@u÷ù=ÙcÀAhr° ÅÀ8סÙÙû‰À:ø
ºÓ¦?ðofÈ61@œ4¡rV	@mŸ€8t'¿évq¡Wþð¿Ñèß	Ü5¿ç­o÷¿ì¨Ð%Ǻ¿UNASNonenone?‰óѯ<"(?'VÐFøÐ(?ï˜0¹Cw?'VÐFøÐ(?Á%ëhŠ?Äõ€Z=þÎ?붿E%þ?Äõ€Z=þÍ?ÃDݶØã?²•ä½_hL?ë.È IÈ?²•ä½_hL?Ñ(µ>g}ª?³¼ë°gå?çk¥`ÌA+?³¼ë°gå3FGL J1749.7-0305@6ú¾Yl'à@(o:¼"peÀ9,AˆaÀ; ¡`7x?Æëñ•®þ[@ß9Xç!ã@fÀ_ñ¿ë Þ®ÁÊ¿Õ@ÆÚ'w¿ç‡½;èÁþ¿íË !³ƒûUNASNonenone?¼|Íx¯àÕ?¿gYf>ŸÒ?ìpfPêæ?¿gYf>ŸÒ?ëvvÎ}?ÁÛä½Ê²î?ÃãÞ&$Æ?ÁÛä½Ê²î?ÝìyýU/?¾i•Zëìà?á	ÃrÕh?¾i•Zëìà?æêY'î?¼@"f.j1?Ò+ÅM°#×?¼@"f.j03FGL J1750.9-2220@ö>¶5@ðï ´«nÀ9³Ët9À:oóþj¿ýQÃI@eÌ@AþíÜ<@¤hŸÑ—¿æ6ÈG'¿íáÇï~Ž·¿¯¼ äôXN¿åO¥&À‰UNASNonenone?ï¾Y/Fß?Š	ÄqkjE?€i´®H'?Š	ÄqkjE?ïu æHIÛ?²¿ ò3™?'[ã6öÄ?²¿ ò3š?ë‹ÑfÖÉÖ?®‡"ðt.?Áкd¤Ø©?®‡"ðt.?ïÿ·ß;?I8'¬?>ñ:œá?I8'œ3FGL J1754.0-3321@vQú¬Ùè>À'å=ÌÀ8çj"ò¬À:·D[y£Z?ò¹ÊE
@­\7äH@K?ëÓM¿Ëý4±ëþt¿êGVù'¿àÜÔ2Wý(¿ìý‹UNASNonenone?Ú9¸Õçy?̜Rø#eh?âã#±D?̜Rø#eh?æÀÛ¦§<}?ÑßiÞ×I¹?Ò~H²±‡?ÑßiÞ×I¹?×µ0×Ô9?»ŒÔH'?ä%gž4ã?»ŒÔH'?ä£ú%sx·?»QþÈЄÂ?Ö¸µ'?»QþÈЄÃ3FGL J1757.8-3126@vsC•Àv€®ç	À8ÞæïÁõÀ:¢MùÇ?ïÝæ"bè@
6ÐfŠM¡@[,å¾`?ýGªí¶ž¿é^¡i5Š¿ã¹ÛGR¿¿ìÔ°Å@w¦UNASNonenone?°¾	cvÝ?¶©1v@>?íè<¾Ó'%?¶©1v@>?Îe&)
H¦?Ð*@W?èf¶u½m×?Ð*@X?ÐxE¿æ"5?»ì'AþN?çÃÝ µå?»ì'AþN?ϽÀÊA³?µ¡Z¨èl?èÍo";?µ¡Z¨èl3FGL J1758.8-2402@á•a%´Å¿¦7½D†À8c˜¢ù"¬À9æ×5??ðíäI–!@Yi}È?ÿæÀ'¢Ü?辶ÈèLì¿ç&k
·p¿ÑgîõX8¿æžºM8UNASNonenone?à'ÆÅ 'J?Ï
h£\kA?Þúrt¿±m?Ï
h£\kA?âáéáç^?Öޜw˜_?Ú<,<1ÛD?Öޜw˜_?ã
¯·\£ü?¶×Rú¨èS?Ù䠑F¸?¶×Rú¨èT?ë V‹—e?Âj™c½OO?Ãû~¥Ñ¢h?Âj™c½OO3FGL J1758.8-2346@ÈëÌlU?´Ê¿_»ýÀ8^@'7|À9Ǩ§b°?ó›÷Aë]@
Üçl`Px@£¬ "Úƿ©ço?ï•ç·B¿äï]+»Uè¿ä&VÅ£RUNASNonenone?¯ˆS^•?¹ø¥?îzΚ°?¹ø¥?¯0aåœâÎ?¾ðíëzß?îùá¦1Ó?¾ðíëzß?Տ¥À¼Ñ ?¸Z+«N?å8-¡—p?¸Z+«N?É		u%Ú?À9N7´?é½½¢¶¸	?À9N7´3FGL J1758.8-4108@uì²êòÀ ÷W÷7ÚbÀ9Ÿ"!°SðÀ;OrSÍÝ?ð9ýŒÞ[@¨¢?¢§@ÓÙ m2Þ¿ÝÔR}%o¦¿›÷Dg"¿å÷
€û¿åm|^ªöUNASNonenone?ç2xCL›œ?ÉOB'}¿8?ћyfÈÉ?ÉOB'}¿8?æƃ¼Ø™¸?ЩŸŽ Ýo?Òrø†N̏?ЩŸŽ Ýp?ç'ô	ÐÒE?¶ìZ"=?ÐÚì^[w?¶ìZ"=?ãœ_×7å?³xÿ˜à?ØÇ@Q'ü5?³xÿ˜à3FGL J1759.2-3848@v0@9«óÀ´ãy·|À9qiiP%²À;ö¬š'^?ôÑïK|Ö@×ëϜ`@ãéÿ"S?êužåÞÁ—¿ÞWí',Q†¿àRcz¬L,¿ïÿû)pU—UNASNonenone?À†y1l?ÈÖpO?ëÞx¡³»å?ÈÖpO?!-ä¥H?¦]ŒÃÂyÜ?ï~÷ÚÕ?¦]ŒÃÂyÜ?¼B¢ik¥6?«Jä4ë·?ìw«²Ò‹X?«Jä4ë·?²ù…*ž\? ‹ð˜:&?í ÏZ¬4? ‹ð˜:%3FGL J1759.6-2141@dÁr%·?î¾UíQÀ8ªO¨´¿À:0``'çÏ?î4)¼«±8@ò҈"£Ä@Ks«¿ìMÃñö—¿â¦â+]¿â¬Ö²°¿èö® þìôUNASNonenone?´‰{\õ<?¿Elg`)É?ínДa\y?¿Elg`)Ê?ÄT¡¯U?ɓÚõ¹L ?êê×½?j?ɓÚõ¹L ?ÖÜV˜®?¸s—rI¹?ä'Ôý|3©?¸s—rI¸?ӌœÐ®J?¿b¶èvò?æ9±±¨Û?¿b¶èvò3FGL J1800.0-2955?çò–öQ*•À	¼©ïR2ÓÀ8®ñ7æ [À:k¹8›R?ò¦©½S2,@Å2™Û2ì@N5gÙÙ¿Ô­æ¡Îá¿ê²ÞŽ~ˆ¿ë'ÏÐã1é¿ãʎÎ([XUNASNonenone?ÐÈpŽ!Âz?Étef×é;?ç›Ç¸ïÄ?Étef×é;?åxï²dkX?ÓïñNº?Õ ›7)Q?ÓïñNº?ݝ§'¥h?ºšà‡'7?á1,pì-L?ºšà‡'7?Ü_'ÛßÜ?Ã":ÎÉq?áÐlõ?Ã":ÎÉq3FGL J1801.5-7825@sµ4'¾‹ÁÀ8b{öÀ9t¢ŸÒ™À;?Mó¨Ú¿ë)Ԓhø½@ó*ÁŸ@	òŸÅ,Å¿ê[i1¿7/¿ç@.·V §¿æ
Ðl-j¿ãOïáêtUNASNonenone?ïÿ'…-1!?
ù	ûý¼?ž´³·«¸?
ù	ûüZ?ïåÕV´?v˲Ð.?j*ô©~K?v˲Ð/?ïÕB§^‹º?uÓ-:à÷Ê?u^¬Pº"Ž?uÓ-:à÷Å?ïþ_åaîÝ?%µïlyµ¹?*©á1²?%µïlyµ¸3FGL J1801.6-2213@uw¾}~±?Ó|½U`"¥À8ÔQ ˆ6À:1sˆÙ?ㄾ2Ö"@
†ÆÎ[S?ÿ{vÁ'}?ïò"c"'¿Õ89Wd•×¿é'L"5à¿ÃÀdÿðUNASNonenone?ÐèÒZøß?Ï,{*ó'?ç‹ñ–Òƒ'?Ï,{*ó'?åRƒi†ý+?Ԝ.×å±?ÕZù,òª?Ԝ.×å±?á¨*o·#ñ?¸š¥ÍK?ܯ« '¸?¸š¥ÍK?ëÒtìeZ?»A«N_?À¶,Nkþš?»A«N_3FGL J1802.4-3043?Óqº™MÀ7%_5½À9?»vc3¬À:ÞùN59?èÒD–ï@
}XsI@â°À|²X¿éþ*7Œa¿à"…‹ð¿Ñ2©gR»¿çy‡‹ÉDUNASNonenone?íŒÿIˆñ?´÷÷¿	N?³˜·;¸y?´÷÷¿	N?æìÔD1m?ÑúÆϚÆ?Ò&Wwϝ'?ÑúÆϚÆ?ë4ëù'3°?°suq)ƒâ?Ã,P÷1=?°suq)ƒã?è$«8?¿eâ"Å2þ?ÏoÍS¯'?¿eâ"Å2þ3FGL J1803.1-2728@	ÄÙÆ°SÀ³#»ÆëÀ8õ	¾ºÀ:ŸŠÙv0?æàK£R¼!@0î™Ñ!ñ@°yݽ¿èBšëdx·¿ãðd@"»V¿ç
zÎ
¦¿äâlÊ갟UNASNonenone?èˆJS!?Ç~xùëv?ÍÞ×ÿª³?Ç~xùët?ê='"L?Ê??2mÞ?Ç¡õîϺ?Ê??2mÞ?ã'›t8?¾iÁä"=?ØûÂɏÏ?¾iÁä"=?èä²(\Î?¶D_'#>S?Ìm7^ŒÇž?¶D_'#>T3FGL J1803.3-6706@tmã}é9ëÀ4^,ýxÀ9†‡OêùÞÀ;§âïÙ?âÀƒ!w@ΰýŽa@»_ÛÝ·¿ãâ݉¢D}¿á-0K'Ï¿ã®1]›¿éí.ÔßôUNASNonenone?åß¼¨¿/®?Í$zOc|Ì?Ô@†® ¢?Í$zOc|Ì?åïßâ?Ìb*|€?Ô AñØx¼?Ìb*|€?è|,[¦Œ?¶˜Î^Æ?ÎN'ùeÑ?¶˜Î^Æ?ål'»Q?´Å/;ÂiS?Õÿ'°Þ‰^?´Å/;ÂiS3FGL J1804.1+2532@IÕcíb@5*ò¥¤i×À9Ä*lEÀ;˜€LÁy²?ï¼ú@ÝÂ2…@µŸe`'¿äë]ÃÌëM¿î›"rëÚÚ¿Â5¤"ÿY¿ïÿÓÉ&‹@UNASNonenone?ï£5ù³H:?šŽå.Øåæ?‡2"-ñ{?šŽå.Øåæ?ìÉuÓ{1m?Â(Tm÷i?¹´Qd&t"?Â(Tm÷i?ì*!CÍ/9?©òÏÓçü¥?¾®õᖆ5?©òÏÓçü¦?衅œ`w?Â>âa£w?Íyëݎ~'?Â>âa£w3FGL J1804.5-0850@3¦Rz WŽ@ôº"»äGÀ8¤3¢Ä»†À:¿b֎í?ÛÆ:{?Ö@§!lŒE@þÏ@šyé¿ìâAa&ê¿âÅÝCVZÄ¿á"
ëiß±¿èÍ/UNASNonenone?ïê´jf? Ó¤©ë…?žb©r³.X? Ó¤©ë†?îâoS?D?²g¹Xáð@?¡Ù
Ì¿3?²g¹Xáð@?ë¾£E«?®¼åÌÊÄÈ?ÃÝréSÃ?®¼åÌÊÄÈ?ìø¼;];Ê?¦UŠê•¥ä?¸:%!´?¦UŠê•¥ä3FGL J1805.9+3407@NGæÿ}ú@7¦êÙ'N#À:µ7"Ñ‹À;£Ò$ûb?ҜkÒGFL@3úkU9@Êî «†¿ãå~'*ð¿á©›yÙ¿ë‹<7yúÿ¿ïüO¹ÑlUNASNonenone?íûÛDfwY?±×•Ï(%?°!%ÜÌE6?±×•Ï(%?íïb"ŠÒt?±šŒÃcl?°"îë©l`?±šŒÃcl?쌂e‡¦˜?§íukþÆ?»›ìÓÂËB?§íukþÆ?éæøš'¨U?³¬£¡35#?Èd•õ^«?³¬£¡35"3FGL J1806.2+2744@K"BJ'k@5ƒ
®>lÀ:w`‰­"À;¢bAQ?ìßôi@X@!eIZçØ@ÆlZ(@?ÀkQF;¿í@Y?¿Õ¿†nª¾Á¿íÞES­b`UNASNonenone?í_DD˜6¾?¸›èہ"?µÝÛ>J?¸›èہ"?ëˆÜB(Ëþ?ÃFy½É˜?Á܎÷\Ð?ÃFy½É˜?è›_'Àô?´÷/ CƗ?ω'ƒ`ü/?´÷/ CƗ?ãg#qC?Áé·ïӗJ?Ù1¹yÅ?Áé·ïӗJ3FGL J1806.7-2451@"K3ÚùÀî['ÍÍÀ9;ofÀ(zÀ:ywÞ]îÉ?èÞÎÆ2e@
×Tª1@«å÷1¿é–´~¿áP²êšàc¿ìÖ;Ÿpý¿¼ß¢-«¤UNASNonenone?à"ŽhÍÃ?ÎV[%Ly?ÞØã.dyÒ?ÎV[%Ly?éÛ

?ËO'$Ëy?ȓ˗×Ïö?ËO'$Ëy?âˆ)‹¨?»¾­¦§1æ?Úï­Úéô®?»¾­¦§1æ?ëeEžü«?¼odé¾ú?Âjé"
Sø?¼odé¾ú3FGL J1806.8+5346@Ty
®>lL@;ÿ:Þ"_¦À:#éõÒ"À;ÛzMÝÙÀˆ6Pôå@Ô(ú@@… =w°¿å«lˆûwì¿çÛ×ϊAb¿êy£¢†þ? îÒº…IUNASNonenone?ïÿcÔ½é?'JØþý?…h]â»
?'JØþÁ?ïÝåÙ» 8?|3ÿ
۩?q
"oãÛ?|3ÿ
€©?ïÏl˜4Àa?v¿ /ÉxN?xI³åŸÏV?v¿ /ÉxS?ïÿû÷->Ç+,;G>À#õûJ‰˜>Ç+,9P3FGL J1808.4-3519@vM—á2µ_ÀsV?§µ¼À9¤qJÅöðÀ;8ñ±ˆ¤?ñ/áo@
È-â¼MN@xÀ`'̤¿äñ-Çl¿á"ðŠ—=¿åp-ÇZêT¿ïýÁÜPDÞUNASNonenone?®[ÔÖNº…?´ƒó¤Ç½z?îB²›X?´ƒó¤Ç½z?ˆr¤Re?Ÿâ".ûÒ:?ïÊ5n¶l?Ÿâ".ûÒ:?ѐâM˜ÏV?¶'£ÝŒ?ç7ŽÙ3˜U?¶'£ÝŒ?§n܊¿w;?'>¶§?î‰7TŒ?'>¶§3FGL J1808.4-3703@v52€ñ,(À `€ù£wÀ9ݛڼy˜À;^G;'ô;?òÁ1c$g"@Õ'X3¼@‡¿¶cÕ¿ÖáY«[Ò¨¿Ü× ÕË¿çKbã鸰¿ïÿmäñUNASNonenone?‹²ÈlDµ?"ސ$­?ï'4ÞNí,?"ސ$­?›¨±XÚT?²+æ"R"Ó?ï"ºw¥9-?²+æ"R"Ó?À{aUÄ?®ÇÀ 7(–?ëá;'ªŽú?®ÇÀ 7(˜?®êÆ:´"õ?˜;"×´­Ë?îSœT¶°?˜;"×´­Ë3FGL J1809.0+3517@NýéÀ"š_@7aæÿ}úÀ:&Nw\WðÀ;¬GðY™Ï?±|a9L@
ƐÃ/@‡þ¡e–¿ä2‡»åc¿éÊ'•_!¿ÝÑnµÈ×Ó¿à¥R­29UNASNonenone?ïþ™¦Ô?+âž~
…?&ež'¾öê?+âž~
¦?痢é֛?ù'>}Oç?†…ŠY??ù'>}Oæ?ïžY³µé?ƒÖ—hP?ˆi»"…Ä?ƒÖ—hM?ïL>Ϟ2?‡Í&"È"z?–x=9¸?‡Í&"È"z3FGL J1809.2-2725@S*I¥ÓÀ	í9SÞ¤À9X*ˆiÆmÀ:Ññd[Ê+?ìJõA` @þ~^@x›_lw"?ïÿW'rúb¿ì>Úcì¿֡Nõ¿ç[k•>.ÿUNASNonenone?ì÷fE(.n?¾ÏÇ
ëü?¸DÍÖ¾Œ"?¾ÏÇ
ëü?çYáp±ð?Ò,îZÉ?ÑL=ڜ ?Ò,îZÉ?æÜ¥GöcB?·ÑèßT¾ü?ÒFµp9~?·ÑèßT¾ü?äâÜ®Ú?Â)Ãrsì?×ÝÎ:F¢L?Â)Ãrsì3FGL J1809.2-2016c@$]7qÁ
¿Óï]ŸˆÀ8)SÂóáÀ9¬†2´ˆ2?à¬Dh@
í÷ßõôc@›&@©¿ãVA`{‹¿éÞ)å¿æ"=Y|Èþ¿æÜuþ†GUNASNonenone(?²³°÷z?ºö/Ðŏ+?í½lI‰á?ºö/Ðŏ+?×2ö;¤Û?Ҋ[
3´?äfñ"â-'?Ҋ[
3³?Ö>ocsI\?¹ùAv¸ü—?äàÈNF[S?¹ùAv¸ü—?ãÑ¢-\ú_?Èúˆ$›…&?Ø\»¥FB?Èúˆ$›…&3FGL J1810.7+5335@Tq´ör2@;h}ˆÁÛÀ:|¶ýW¯À;ÞH'¶þ.?í&/Úc8_@
Ç«äÊÅa?ü{óI"¿ïþ§UCÿ3?ïôù&Ёì¿ÊÖøwG¿âOEèÂv³UNASNonenone?ïæ˜ÐÆk+?mL	P.ÝU?ig/9"ÔÅ?mL	P.ÝQ?îJ²^øö?°j	"@õ¤?«_´Úp¬?°j	"@õ¤?îÂx:{ãò?˜œ¸Ûr!÷?£Ø|XAÀá?˜œ¸Ûr!ø?êâìô9?¶vÑ®¬!?ÄwàL/Ï?¶vÑ®¬!3FGL J1810.8-2412@¦ÚhµÌÀ2J…_OòÀ8Œ°±
S¦À:,ñ.?õƒ-œpc•@'¡ùxƒ@—1@"ÅŸ?ïþßF]C¿èÏÊ÷›¾ž¿çHìÏ¿é/ّ×-yUNASNonenone?¶½òHæò?ÀåëÀ ?í(\á¶ã!?ÀåëÀ ?ã´í \õ?Ó`¼…™¡j?ؖ%¿GÄ?Ó`¼…™¡k?ÑÁ§Ÿ–Ìã?ºÏLÎF?ç,04™Ž?ºÏLÎE?ÜÍ¿-`Á)?ÄkÂcf?ᙠiOŸl?ÄkÂcf3FGL J1813.6-6845@tY+jçÕgÀ5ؖÝ&·$À:0ÅJ!ŒÀ;¸¨Uôÿ?ë@…ñh"ñ@…ÖVÍÂ@9þgú?º'¡0Dt¿ãn¤ç?ó¿íDTd ¿ßHQŸÒ:UNASNonenone?ìV"–»–?Àã:·åŠY?½NëJ'ãQ?Àã:·åŠY?íÖr¥'Í¿?ÀùB‰÷'‡?±LjÓé'?ÀùB‰÷'‡?é46‹2§?´J©'g,?˃/%Ó5d?´J©'g,?æbºHÖ«?À´enæ?Ó:‹õnRª?À´enæ3FGL J1813.6+2820@K¡rGE8ï@4,ÙÆ°SÀ:0"t¼jÀ;¯M†›¿¬vä"`@
EiÁƒ@§†€b;	¿äj4Z`ÚÇ¿è=&ÃpX¿Ù± ˆ¿ã%ü¬,'UNASNonenone?ïþiÖmò?,½‹µW^:?)n¢™ ïÑ?,½‹µW]ý?ï¸o9k˜ô?‡ö苟)×?ä1¥Ã?‡ö苟)Ö?ïģа+?z¼4$ÉNµ?}þ.§ê?z¼4$ÉN²?ïtì'‹®™?ƒâ¬}GGË?'b{Š,ô?ƒâ¬}GGÊ3FGL J1814.0-1757c@)ƒÅ›€#§¿Æþ§°³'À80RÆvÀ9ŸY—K
À?íð}ø9žC@NÎLBy@s&@©?ïþ€ªú¿ã+…Æ9F¿â—y';|-¿íb=/òr4UNASNonenone ?¤EÈúë´Ó?¯†…j?pQD³?¯†…j?Ô`—ݸçô?ÔYNoGì…?åÏ´#Œ?ÔYNoGì…?Ë#÷­ïYA?²_œ©\Ä5?é7")°?²_œ©\Ä5?áìÛ/¢‡?Êê"aI?Ü&IÇ ºò?Êê"aI3FGL J1814.1-1734c@*5¤i×4/¿˜¡©¢?hÀ79™J¿@óÀ9tõɯâ?î:ÕG*ó@*bÐYÊ!@_R`u
Ä¿äüoÞùäͿ菪î^J—¿éÔnÆ $¿éK;eé#UNASNonenone`?´`
Bò"?½Î"Θ?ísþ·®A¼?½Î"Θ?ƙ†Xl¦?ÈÁ`ƒ€Ym?êYž{©ä×?ÈÁ`ƒ€Ym?Îr¼WFÉ?º¾ËiH?ècPê9nN?º¾ËiH?×&ä¯î£¥?Å©R¨û՘?äl¨®-?Å©R¨û՘3FGL J1815.1+5919@VÛ"Ðå`@; ¢G'ÝÀ:þ—J4À;Ñ-åìXƒ?î6,óå@ÃQžƒ8Y@‡ÿž[J¿å¾rMi.¿éWȄÏÄ4¿êTq£J6I¿ïý›¢ÄvÎUNASNonenone?ïqÕ{ÃëX?•;[ç[¥'?'ÅP‡'"ô?•;[ç[¥'?âYmm–‹¦?ÎÃ?@K\ó?ÛM%$Òè³?ÎÃ?@K\ó?ì_
f49?ªtØ<à?½"Ëö^3?ªtØ<à?ÐŃ÷Âç/?µÕº>ž–?ç>Œh?µÕº>ž–3FGL J1816.0-6407@t¥e¶™…À4"ÕA"ÈÀ9r"#—µÀ;¤mµ@æ?æféšõ@~6QJËU@UŽ >¹Ï¿ã©WD_€n¿æX\ãZØ¿¿æÏÜ°´W$¿ïÿ:g|]kUNASNonenone?ëYO'ª?Â>¡w'ή?šËcU?Â>¡w'ή?Õ@Ü2–Ö?ÎMR­h
?å_ð'æ´–?ÎMR­h
?êA	wé0?³0k%;Õ+?ÆûÚ#€[??³0k%;Õ+?Ùҗz}P?·K'mW>?ã´BÁ7Ø?·K'mW>3FGL J1816.2-2726@ŒS£C^À€`îWaÀ9Û6òÛÀ:òyùK?ÀõßÐyn@ý¾ž
ío@aHu«ÿ¿çv¶ÑÉó¿æÙ;®_ù¿Þ™±¾Jö¿íLøÿZ¾'UNASNonenone?çøBQ0Ë3?ɂÜÞtÜj?Ð{]žiœ?ɂÜÞtÜk?é|½j8'?ʃÌ0è‹B?Ê
WÍø?ʃÌ0è‹B?æËDÛæ?¸^2ôc}?ÒiÁvH3ø?¸^2ôc}?í	àœõ@ü?¬S¨koì?·°ûUø&?¬S¨koì3FGL J1816.5-1145@2}	¾º@ŽœæU4À8x‰žyÓ+À9ùÛån"B¿ðfÅê/‰0@8Lø1@Øbà¿ã¨ÝF‰¿ç¿©ò	ûµ¿émwâß¿âaÚK̘[UNASNonenone	?Üçf<œýf?Ïç"1²#?áŒL᱁M?Ïç"1²#?ïs
Ý´²?®úzÔè"?'žDI|	œ?®úzÔè#?àçÀñ‰?¸ /@å-ó?Þ0ÀíÍ?¸ /@å-ò?ïíŽ{©Z×?o}$¬¡£Œ?bq"V¥(z?o}$¬¡£Œ3FGL J1817.3-3033?ÿÙÞ7X\À+àÞ҈ÎÀ9ÍâÀTÀ;+	¾º?½Åƒö;±@'mÖÈ#E@v?@\¼o¿ãª"
õZ¿èStM9ſ冕l¿ããPM[Ž­UNASNonenone?ïÖG#q?yRlŽ¡t?tÜnGpñ)?yRlŽ¡t?ï6¥ýkT?«é-ª
?žy+@R•…?«é-ª
?ï
vP›ß?–ÊCÎ֎—?ž±5ì"?–ÊCÎ֎˜?ï^íÚiz?'è†>Å|?"D²Ð¿?'è†>Å}3FGL J1817.7+2530@Jh'¾‹Áj@2Ma€M˜9À9ï6¥®zÒÀ;Œo[Ømë?èä¥c§DR@•·+о@¶Ÿ¤n¿Ý3X$·Íë¿êù^QÊ¿âoµÅý®J¿ïÿµš1DUNASNonenone?ïèTÛ?p:îÌbÕ?gì«à<eb?p:îÌbÕ?ìdÅm
`R?¾bÚt^HÓ?¼Ùԗ"ýo?¾bÚt^HÓ?íëXëÌô?¥~³+P?·˜¥8¡˜b?¥~³+P?ãŒzn–?¼êž+Ê[?ÙÚç#âÓ?¼êž+Ê[3FGL J1818.5+1320@D§¨ÖM@*|õn¬†À:&ÕÖ`ÊEÀ;Œ¥ÉRÄÉ?ëòm–¾@æÚâå@Š`@²x¿éžˆ‹v¸¿¸×mÌ ª¿â¬"ÀcT¿è'¹ø‰¿UNASNonenone?í«c!?·_7¹n±?·w|¤æù?·_7¹n±?ç/¬ñ‡?Î6™ï˜<?ÑË §Èò?Î6™ï˜<?ì~U ?©àð:h?¼
WÏÏï?©àð:h ?Ø5ïâ?ºåR='þH?ãåñüs?ºåR='þH3FGL J1819.5-2045c@%ˊ~s£fÀ"Í*1,À8÷þ×0À:‡Û…Í3ûÀeVWz?@qÛøòÆ@¥"úI¿ço-5B¿êåCÔɤ¿àLyõܲë¿æVÈ¥1
¥UNASNonenone(?ïªy…=§q?áÌS0B^?…až°–#å?áÌS0B^?ïr:篚?ªˆgáµ¢?'¸£
¾Ý?ªˆgáµ¢?ëàŠØPP?®"÷ÖûÔ?Á¼}Ԟ¾Á?®"÷ÖûÔ?ïÿÿ_éX>½#VÚ¡Y>>œTÕdd>½#VÚ¡X3FGL J1819.5-1345@1mÁ¤zž?ä©À°ñÀ7éÞ(>ãkÀ9Ù)Š=D¿óÐý8zoÞ@jÔÙ`®ì@Ò$ ›«î¿ãŸ"›
jª¿ëCS‡ªó¿äêžB²¿é«F{©3UNASNonenone	?í7>eZš?º¡åÎs?¶F×%+3?º¡åÎrÿ?íFHLD?ɔí…i1?·Ï
ͽì?ɔí…i1?æ'[V<Û¢?´•FCµÕ?Ó±IS†H¼?´•FCµÕ?ïûšBR?TsQåé=0?C¹–ö·º'?TsQåé=23FGL J1820.3-1529c@/Nñw§Š¿Õê'nQí3À8>ö%‹ªÄÀ9z«Yµ}ü¿ý%1¸^Ö¥@uÌKȀb@¥5À9ü¿èˆÑ§ÊVG¿é-XQ¿âA¥WÏ¿ìH	èrUïUNASNonenone0?äّkçs?Î{ó<ÁC?ÖLÝÝ(1?Î{ó<ÁC?ìðC¥>*?Ê]z>g@¡?¸}âÖ¯Ô?Ê]z>g@¡?â²0"y~?³ÔjTÈ|—?ڛžÙ
ä?³ÔjTÈ|—?ïóXù¨}?vƒ%×2XÆ?YN¯ýÓ?vƒ%×2XÆ3FGL J1820.4-3217?ç•3­ÁÀ TMryšÀ9^ê䭔À;2;Yrb?ó/ÂÖ(ì@«©Ô¥3V@À]€c½•¿Ü]©¡³Í¿ã˒ìgƒ¿æ·°ÌC¿ïÿfh¥ìõUNASNonenone?  JW/Ôì?§<w·ð?îõûZ²?§<w·ð?²[è~bÛ?»q
Óç
?í¿´'ð3¤?»q
Óç
?À–Y"Ž¸?­³©+ÂîQ?ëÚižÿÜR?­³©+ÂîS?ÂônÇ?¥zuWÕy?ëBûýäX?¥zuWÕy3FGL J1821.6-1436c@0'j¨ëF5¿É'îz°À7ÕõŒ·_À9±Ããïÿ?ì‡õÁþ)@í{µƒ@S<À¥¢?ïõŠZCÝ¿âU¤Ÿ‡d¿âý5ò°P¿ä_æãUNASNonenone ?Ö\p!é?Î'¢];œ³?äÑúsÇï
?Î'¢];œ´?ØƵ;s?Óæ¨)ê6?ãýÿœ¥bF?Óæ¨)ê6?ÚÄLS‹?º²Q~ák?âôYõÖ:?º²Q~ák?á(Ir³à?Çm uG+?ݯm˜?Å?Çm uG+3FGL J1821.9+6636@X"LƒfQn@;£ŒSâÖÀ:rˆšmÔðÀ<Iqc?äEO¶²ÀB@ð`™ËX@S—Á¼M¿ëóL´ÓK¿ßuÖ¤o"¿Ûô¹"'¢¿Û
`ߌUNASNonenone?ï˜íž)(5?'%Cä'?‰Ä˜uµò¶?'%Cä'?î(@ùïZÅ?´·ó1|ÄV?­{ða
Sº?´·ó1|ÄV?ïJdôñü?"UÏß·ô*?œ–³aaÀ‰?"UÏß·ô*?è;8%|q?»×"Ñ5?ÍÃj>?»×"Ñ53FGL J1823.2-4722@u°í(ŒçÀ.R‡;©À:И3hÀ;ŸÁ}ä1m?ô)Óݍ9@¬4VHáñ@TÿÀ,³?毐c1u¿Ìŀlßk¿áq™ô™€«¿ïÿô›.*qUNASNonenone?ØKÈ¿j¼z?ÔF˜ÆÔº?ãÚ J¡Ä?ÔF˜ÆÔº?¥¾}•=?¸‰6¦ eè?î®4&¬.?¸‰6¦ eç?Än™Œ²F?±£‡ãLeÊ?êäY¿ÜÓo?±£‡ãLeÊ?¹qOÓɎ®?¡˜V$ut?ìÑÖ†Î*?¡˜V$ut3FGL J1824.2-5427@uE	k¹Œ~À2
cÇOµÀ:WL0À;¯rçԐ?éƸ	µû@}ò

@¥ØߪŸü¿ãYÝUtëS?®ì:•ñý¿å8S¦ù²¿í"vmUNASNonenone?×P8ñW¶ç?Ë%Š
ßæ?äWã‡T$Œ?Ë%Š
ßæ?áٗ¶Õx=?ÐÇÊðkÉ?ÜLВU…?ÐÇÊðkÉ?âÂýž¡ú,?¹ºvÑ7?Úz¼¨?¹ºvÑ7?àÇäÈ–?µÉ8_•Î½?Þp7ÐnzÓ?µÉ8_•Î½3FGL J1824.3-0620@82Ø]ú‡@©U´g{9À8‹'®›‰^À:š'Bdÿ^¿õù}d¯­@
éGZÝq5@òø‹áu¿ë(¡–­¿áҝç˜;¿ÊwÃÛâi¿ìè2a"³UNASNonenone?ßôpPžÆù?І<§q=Á?àÇ×°œ"?І<§q=Á?l	Ó?¤—Ú6ìr?Žüäý‹b?¤—Ú6ìr?åØ¿Ï7q?³±#´	ë?ÕÖN€a'?³±#´	ë?ïòë%ΊÐ?oß³&Se€?Z)´bê_ ?oß³&Se'3FGL J1827.6-0846@6k"Àh¡?óݑ[¶ÓÀ868À:;¾íæù?֘nyé@I—M¹ò@åÎ 3ý¿çAT惤‡¿ã²')Þu¿å·x®¬?'¿ççÁH›`UNASNonenone?ÃB&v¡Ã?ÇÖ~M³5ÿ?ë/vbWœ?ÇÖ~M³5ÿ?ßÁ*Þ;už?Ô¬zŝ'?àjâE1?Ô¬zŝ'?ßr'Æñâ?º¾ÌƒÕ?àF¶œü?º¾ÌƒÕ?èuŒgË?¿È²¹•?Î+ÅÏÂ`×?¿È²¹•3FGL J1827.7+1141@Dd	þ†ƒ<@%	Ž«ÿÎÀ9›iK4ÄÀ;[ C×Æ%?õe3€µòì@
9r&@år?ãoÑ?î4~{ŸÍT¿áp$2íÆ ¿áOþðáT¿ïÿð	V¯©UNASNonenone?Õo%ýøR?Ñ/÷
ƒûÈ?åHmr×?Ñ/÷
ƒûÈ?"
by¹e?¦œSc'G?ïg"ïÜ25?¦œSc'G?Â&«Þ‹ù?¯e¥ýâÕ?ëv{•]?¯e¥ýâÔ?­Ýéu^Ô-?Õ	…פ}?î"!hª½?Õ	…פ|3FGL J1829.2+3229@NRs×Ûõ@2"Ø#B$hÀ9þJÁÅ1ÎÀ;¯Ux™]?ô)ÎØÀ ï@•kâ@H?ìT'?†F¦¿Ýl0%Ú'¿çÈRoò¿ïÿÆ:Gµ²UNASNonenone? íÖ%"^¬?¨ªY¢#?îñ"§º?¨ªY¢#?Åc•WFÛ?ÅsQµ‰:?ꧾª.J?ÅsQµ‰:?Áò^cƒöy?¯ƒÖ!àW?ëƒhgb?¯ƒÖ!àV?¼³,ùïò?¢óªÕS)?ìiš`Üb?¢óªÕS)3FGL J1829.2+2731@Kæe+ÓÃ@0­Å÷Æu›À9lg"cϳÀ;Š¦Bˆ?ðÊÅ~#òN@'‡µÁms@õЀ5šl¿ãÇa/Åæ¿êbà[09¿è'íþÔ:¿ïýó®Á|•UNASNonenone?íÑ>_ð?´S-r&j6?·Iw>
ƒ?´S-r&j6?ã.·º¤m?Í1(~öX?Ù¢Š·Ù'?Í1(~öX?æP)NºrÒ?¹ûC:IKÈ?Ó_­b‹\?¹ûC:IKÈ?ÒÌ¿Õe^?±""Ã9Ê*?晠M@Q?±""Ã9Ê*3FGL J1829.2-1504@1ÉêpLÀ`QyoW§À9$¤úö¬À:ºÊ9t•Ô?íE!@R¼¢@PԃÐZ?ù±Iß/¶¿ï\ ރ׿Ç2"J¹¿Þ†$æÙR¿Ì­ÞJÄUNASNonenone?ê¬j˜q x?Å>"®ãèÃ?ÅNUž;~!?Å>"®ãèÄ?èÂA®MOK?Íë\?ÌöùFÊÂÕ?Íë\?ꈔÇ~?¯Ógº2º?ÅݯŒâ§?¯Ógº2º?èÞ x?¿pUòÄ?Ïü…šô?¿pUòÄ3FGL J1829.3-0135c@<ýæ>Ž@ÀgHäu`À8É2=jÀ:hƒwe?áŸ4eã3Á@
¨×z$ß@JMà]£I¿Ñ-ðŽHÌ¿ä¹ï[ ˜¿ãWìEÒ·¿æ¿ÿL¯c¹UNASNonenone4?Á)hÅÕ-i?Å
0T%?뵥Ί´¦?Å
0T%?î^j±Î?».+Ö0~?®:Tã\?».+Ö0~?á^ŽÉÜ·?¶Ü<¨ÖT?ÝCúâlF'?¶Ü<¨ÖT?æo­'z+?čHwÖ?ÒÅ ¤ûª?čHwÖ3FGL J1829.9-0203c@<¥£Â‡è@°ò¿-¨À8~MZü¦À9åÈÂ|ó?è˜è…K?*@©ˆGØ%@åŸ×vI?ì\±àüôL¿áJ~]ö+¿áBö\"(ç¿ìyI{…B±UNASNonenone ?ˆÅIUƒ?˜H
@Õ?êÛîª?˜H
@Õ?ä:jÑÑÃ?ѓSwZå.?׋+Î\\y?ѓSwZå.?ÒM=îßuÅ?´£H'º'?æÙaE?´£H'º'?Õèw¿ÎïÑ?āÄ+Û?åÄ ˆ?āÄ+Û3FGL J1830.7-1630@/Ò¬Ùè>BÀ=Šú`"À87 ޜØéÀ:‡ºÿDï¿ÿ˜!<Ю@"ˑ¹Pn@ƒ>@'|¿éôÉwq•]¿âa¨ÀÂÂ!¿ãèH¿?#4¿è€¾­`‡UNASNonenone?ê'Íqƒ?ÄSàÙ`?Å´Ê9ó­ü?ÄSàÙ`?ï‡Ò,Æ?°úÊk• z?/ºnGH?°úÊk• z?ç‡:¥føý?²Y?¸Ièœ?ÐñŠµ2?²Y?¸Ièœ?ïùëRë?[ÆD•%?HSâ´Qû?[ÆD•+3FGL J1830.8-3136@՝CrFÀ#®ç£è`À9·ÙfhÀ;TæØÍ®?ìCÓU–Ï)@
®ññÊ]1@€®_ybB¿ßu¥Ô:X¿¿³ý!£ê¿æ+x±Â…K¿ì8BáòUNASNonenone?—#$0/gÂ? âY¤k?ïFæÞ~"Â? âY¤k?É%´ë!ŸÆ?Ì5@›Ì™}?鶒Å7˜?Ì5@›Ì™}?ק'‰Ø?¹*(!…+'?ä,xô·;?¹*(!…+'?ÐkÊE]'+?¯\+EÛèÉ?çÊÝQ6ì?¯\+EÛèÉ3FGL J1831.7-0157c@<ðÞÁÁÖÐ@źcdÀ8U["¤À9›hýð[GÀ6O†{×@
#nýcÃt@Q¿Š¿ã%ïÓ·ø¿ìxÌwí\¿áœºBÜs‰¿ã–σ$UNASNonenone0?çÇciÖ?ÊP²´ë?Ðq9á,S?ÊP²´ë?ïólŠÌ›?±Ìr?Œƒ$ÝLÙ;?±Ìr?æaÅd/?´‡!CçÒu?Óÿ<u7 ä?´‡!CçÒu?ïý0^àHÔ?Q—Ûµlt9?6}ý¹]ƒ?Q—Ûµlt93FGL J1834.8-0630c@9?î¢	ª¤?ænø`¤Z"À8í^<Ì9À9Øî
5?Ñ𢐟[6@¬fjÃl@²m?ôa¼?ë S0ºÄ¿íö:"`L¿Ô=XRHï¿ÛóÜApUNASNonenone ?é Û¹79Ü?ÇËT]/'?É|'#Ž?ÇËT]/'?ç念û"?ÓQ2°U©Ñ?Ð ²¸ÞØ?ÓQ2°U©Ñ?èî50S?³"õu‰'?πG+ƒ>´?³"õu‰ƒ?îï;Ü)$Ù?© ©vŠ°?¡B=m²f?© ©vŠ°3FGL J1837.3-2403@#±©É'†À<µ]D~µÀ9v"´/GÀ;}}?ÕÏ\t@9muÏ:@6tªL¿çá©	=\¿Ü,Ûàæà¿ãQG¯'[ ¿ï}§SÒ¡3UNASNonenone?Á5øVÙ*?Â$4'øz^?ë»òêI¶?Â$4'øz^?á Ô|ۇ?Ó¬ÞÿœŸ?ݾWHñã?Ó¬ÞÿœŸ?ÝÖ¶e?Á×¢Ú¨Ô?á¤Í@€?Á×¢Ú¨Ô?æ /|Ÿƒ¡?½|-ëè?Ó¿¡Àø¾?½|-ëè3FGL J1837.6-0717@8ÝÔÇm{¿Ñ0‡¼øCsÀ8Y­N'DÀ9¹÷[ÐL¿ÐÈlåJ`æ@
Âp¡æð@L¶€… '¿ìpÑVýÆ¿Ìö%°,œÛ¿çÓV˂Žª¿ãËy:{žUNASNonenone?Ø2Q¿2RŸ?ÍÒú´$b"?ãæ× fÖ±?ÍÒú´$b"?ç&<'*W?Ô?µw!%\?ѳé†Ý«R?Ô?µw!%\?á¥K#4ÈÎ?·_¾×É
t?ܵi¹–nc?·_¾×É
u?î\¯€×?³Ëhz6•Ç?ª>_•ò?³Ëhz6•Æ3FGL J1838.1+3827@PΚ¿3‡@2åxåÄëWÀ9Ù ~(ØÀ;˯é(¿èCc˜D@›@ññP@̾@Bo¿é‡ŸeØÄI¿å;qv¡U¿æ¹˜ÿ"žÏ¿ìÍÈl¸2UNASNonenone?ï?&‹œ?››'dÝ*Ò?œø.Œ®?››'dÝ*Ó?ïT|z[-¾? ƒÏ:-»?•pp´šH#? ƒÏ:-º?î!ñô໑?Ÿ8B>¥'Ä?­àà±ôFÜ?Ÿ8B>¥'Å?ï‡VÉg4'?‡|ºûÍ*?Ž*M¦2ßy?‡|ºûÍ*3FGL J1838.9-0646@9zTæâ!É¿ÔAKdWmzÀ8:úêíIDÀ9ýèwM>?ÓS–=w7x@RQR-q?þ¿>«Œ`?îÅUÌ)'°?ëL¦*õÏ¿ßÙî7D¿åŠ¯nÍ#UNASNonenone?æaË÷ìI?ÌqØ_bM~?Ó<xè'o?ÌqØ_bM~?âBÃÚÞEP?ØU?SV/?ÛzxJCua?ØU?SV/?è*ŸHê&'?³–3^}æ?ÏU'ÜWe¼?³–3^}æ?ì˜D¦5?¿áÕï)Ø?»=ßRÏfU?¿áÕï)Ø3FGL J1839.9+7646@[8›R~@;ÅïbúÀ:po»y¾2À;ÿPïܹ¿Ÿ9%ÑÐá'@
˜áT@ld¿ó¿ã±Š#"ê`¿è¿|¤¶¿âܪ̃¿ï"wõºUNASNonenone?ïÑ?ý»Ç=?†™—îxA¨?w`"`á?†™—îxA©?íø°j?¯d!‹i='?°:ÏÜ°?¯d!‹i=ƒ?î1£Ÿiõ? ò˜üúr¬?¬åÆ9`®? ò˜üúr«?í½*$àÄ?§}©Q£?·®Øùá?§}©Q£3FGL J1840.5+6116@VÀŸ±@8ÙìÔªàÀ9Üuι6À;›¤xð­¿èù+¥þµ[@´D¼­@۞ÿµ¿ë÷&~*8Ÿ¿æ:QB›c§¿á@Æ®-X¿ìªJkßUNASNonenone?ïùΐ%¾?Yђ šd?KÄÅ¿i	?Yђ šb?ïªp‰È³´?uӉ'sÆ?…cݍÓ?uӉ'sÆ?î÷3X({…?•¹Š|z¨? ŒÊ}xG³?•¹Š|z§þ?ïÚÍb½Ê¢?p¦m0Æz?r™N¡¯?p¦m0Æz3FGL J1842.2+2742@LÌݓÄn@,18yÄ<À9'íG–—‡À;|5vÚQñ?ìpRqx#Ž@
?çݟX@!¿mh¹¿ãMû
Qø¿ÖŒtšUè¿ßGDŒ¿ëÙ<\QºˆUNASNonenone?ÐÌ©+ø?Ã]Ø;nÃê?ç™ò«|ê?Ã]Ø;nÃê?ÚØäÕ(e?Ð3Ý=¨R?Ⓧ•|kÎ?Ð3Ý=¨R?à‰ŸGÔ1Ï?¹ŒÜiN¡É?ÞìÁpWœb?¹ŒÜiN¡É?Ö~ÉáœCt?²Åá¬<(?äÀ›1ÞG?²Åá¬<(3FGL J1844.7-1224@56q¬À¦žË1ÂÀ9Lx䓓À:›¸®ã®¿ÖYIŸ}«Ÿ@­5'Þê\@9*Ÿ»Ç—¿ée÷"þW½¿è·×À⯿Դûï=ÿ¯¿áŒë¨ÛUNASNonenone?ï­gì5·'?‹øLdE?"¦ò'6…?‹øLdE?ï>hÂ'
A?ªDÚRÓ*~?˜2ç»·ö?ªDÚRÓ*?ìɘ·˜?¨rÓs‹(?¹³?"Gó>?¨rÓs‹)?ïðV]¤hÙ?ar+þxX?_SD·.Nú?ar+þxY3FGL J1845.5-2524@"á˜kœ0MÀ$(^ÃÚµÄÀ9]ÉòîÀ;*¾áQ¿?äkõö«‡G@
™•}U@N@A0ÿÒ2½¿ã©åÇù¿ç¢I-ÆaÏ¿Ö'ˆvîÀ¿îIt&(ÄÖUNASNonenone?çÏüU`ÃÎ?Ê%m"]€?Ð`U>xd?Ê%m"]€?Ò7T¹\B7?ÑqUc¬?æäU£QÞå?ÑqUc¬?ã…}&B'e?·fg nÔ?Øõ³zÝ7?·fg nÓ?àŸ+N?Â|«ë2R0?ßõþÁÁ©b?Â|«ë2R03FGL J1849.5-0124c@?v«%(®¿ÍÇø<<FWÀ8Ê<ϔ'À9}⊤3Q?ñÂãoPšÍ@ÕÅ©@Dàßÿ.Ÿ¿æ•H\mÇ·¿â‹ƒ&´(¿æÌdÌL8,¿ìFeXäUNASNonenone<?G›Vš#c?FŽDÝûT¾?ïú>jYw?FŽDÝûT¾?§u±€¡Aÿ?³:~Üð×?çõëß?³:~Üð×?±¢ŽJtž¶?¢3÷"¼aù?íË®6±l)?¢3÷"¼aø?Î,ì"ý"?¸èëŸGV
?ëtÄÚÀœ?¸èëŸGV	3FGL J1850.5-0024@@;ò<ÈÞ+?'çT¸i"À7"ºV¨ƒÀ9¦AÂB/O?ôÇW<§Ñ@¦ûjo	£@[?²r"¿Øò‹p¿ŽS¿é™Óêè¿æ†Œµõ3¸¿çÍ`|Ü8iUNASNonenone?±=´|,ÍT?µµü
®W?íØIpzfU?µµü
®W?ÎÁ@÷x?Ì«C
Î+?èO¯Â!ܽ?Ì«C
Î+?ÓÁÉ¢Å#?»•šs€Û†?æp.o?»•šs€Û†?×*mZY…?üš÷»?äjÉRþS=?üš÷º3FGL J1852.8+0158@Alk΅3±?âЀÉ"À77ûº !ÞÀ9Ã~ü_a?òýó¦*v¡@üäõ‹C@`Пëf¿å0ù›ü!¿ê;ƒ[6)¿å²Æç'¿é¬ƒIS¹™UNASNonenone?¡@¶3ª÷?©YK¸Æ®‹?îëôœÎ5R?©YK¸Æ®‹?¤a\H¿ÞÅ?µ™'ö×?î¹ê;t?µ™'ö×?ɒ2Ða}»?µ
oUYu?é›sK砑?µ
oUYu?¿ýµ4?®á1Úê]?ì\)Y}ß?®á1Úê]3FGL J1855.4+0454@Bá
£3v?õ¥+•°À7ÐÌ% †À9ù¡t?íZªŠF"@
:íO¤-@W— mˆÅ¿àï6ð3À¿épJÜ$â¿çNéWпèržïïUNASNonenone?¡Iåç¡R?­aÏyÖÅî?îæûa¡…ê?­aÏyÖÅî?¿Ißq™N?Ç ßûhŽÃ?ìÄß×?Ç ßûhŽÃ?Ð;:i?µ
ÆïKy?çâ@}bòL?µ
ÆïKx?ɘoÿûmö?¹¨¦³K¦.?é™ä$ƒ?¹¨¦³K¦.3FGL J1855.6+0753@D7Æø@B‹`òËÀ8J¡!À:^×òš¼¯?êSrBèˆ@xrÊø·6@Њ©³¿æÚ¯Nњ¿é
X<Ï`¿ãŒ˜qGã;¿ïæ_4eYÃUNASNonenone	?ÁHÂYõ¼Û?Â¥{äù?ë­Ïi'É?Â¥{äù'?ë²Fâ(?°Ñ0Ÿdz?ïx¢mÏÐð?°Ñ0Ÿdy?ؗ¸øé
?».‰B˜i?ã´#ûƒ‹{?».‰B˜i?§Á	Ù(?™øH±0W?îƒï¯ßbn?™øH±0W3FGL J1856.1-1217@6whۋ¬Àf•Ù¸éÀ8î¾c}}ÚÀ:ë´¬D—	?ë«Ë<vJW@ofw®7`@¶?wå¿åíQŠ"̉¿ë7ú&ïzn¿ã€<"Åý¦¿Óm'ÔUNASNonenone?îÒD°iß?«~ýžvh?¢Þ‹´ùb?«~ýžvh?ìÜdXq?Ää(
ªÑ?¹Ý?›"w?Ää(
ªÐ?ê‰4ƒqÍ?±"Zï9ç?ÅÛ/½ò8Í?±"Zï9æ?ë «®?³e,¯K0?ù¡S¹L?³e,¯K03FGL J1857.0-7341@t]9–ûÀ:W/˜sÿ¬À9¦ÃhŸýÀ;¢«%³ð¿ÌÙÑò?fâ@OüÄâ@;z¿ä±ñ¿é€ê&¶v¿élᄌ8ª¿ç؆ð'M¿ïÿaXNeUNASNonenone?ï÷'eù?Uvz\˜?PÝÙ4
ß ?Uvz\˜$?'++?µ«x‹ÝÊ­?¥ugÝME?µ«x‹ÝÊ­?îìµÜ©'B?•îS=¶n"?¡4¢5fëå?•îS=¶nƒ?î—㞯F?˜¾Ç¹Ÿ'?¦Î ?˜¾Ç¹Ÿ'3FGL J1857.8+0129c@A€jüοè	_s­øÀ8+-ß6[ÝÀ9t°/Þ?òö&Û6@
ÌûìJ£@½Óà'Q|¿b7ž¤&ƒ¿ç¡YMp™¿çÛَÀçU¿ë9ì¡î·UNASNonenone8?UEP—ïÁH?Z#×Ô)_?ïõ]W´?Z#×Ô)_?´ì͸øø?¼Ë¯ß¶&l?íbfHààÿ?¼Ë¯ß¶&l?±¸3ÿzœ}?¦Í3Ï÷ù?íÈù€¬q?¦Í3Ï÷ú?Š>]Äs…?·(Ú	ô¯?ë]phŽã?·(Ú	ô¯3FGL J1857.9+7319@ZŽ4@9pJ¥?À	À:
ÍfOÀ2À;ö{í·( ¿ÚÇH¢õҙ@âÎ}Q@'R€«a¿è¢Ç:î¿ìzá%Qü«¿àj$׿ÑÏTŒ[áUNASNonenone?ïýbý¢Ä?B;	©Å?4èéßlj?B;	©½?¯*N?"ò,*í!Ó?‡:ٔ5l‰?"ò,*í!Ó?ï…ùHòFB?‡õ"±e?Ž­Ãno«?‡õ"±c?ïǗôñzÍ?uçØa²ªÉ?|4‡B™‹?uçØa²ªË3FGL J1857.9+5549@Ux+Iº@5GÎÙ‡+À9Î.ümÀ;GþœR±?Òvۆƒ0@Ñoƒñfµ@°uˆ÷5¿é]h»L¿¿íŒQ=pŠ¿Ï||àØ¿Ô¼ÊJ*_iUNASNonenone?ïüH	ªE?E¨µØòK?=¿²­×é?E¨µØò@?ï™è';\ù?™eìùA?‰…ßq(Áö?™eìùA?ïfÛÌçyò?vJQ™I¹?"$†cÁÏ?vJQ™I¶?ïOú«›¯?9¤V?–ªŒŠû?9¤V3FGL J1858.0-5423@u`¢}ŠÀ6­Î|Ð57À:&:ØC""À;·¢Ëq'ú?ésÐ#eØ@
Aå·Tj@ô<ŒAí?ØU$äTÿÜ
Öfma¿é£*—b¿×ñŒÃ%ÜUNASNonenone?é¡ac±=þ?Ç'9n
uU?Ézzq;?Ç'9n
uT?í4wSt?ďžñ[Ò-?¶\GÕd_q?ďžñ[Ò.?é–*Èñ)Š?µVÉUÝ
'?ɧTÜ;YØ?µVÉUÝ
'?äê:À0HŸ?ÂsãÌEÊ?Ö+ŠŸnÃ?ÂsãÌEÊ3FGL J1900.3+0411c@B×u}Zž²¿³'¿ž¢(EÀ8XU±ã<{À9ÈQÎÿ¬ô?♺™Cˆk@
Â/,"[è@ÆŸŽP:¿Ñ:8¦öµ¿è"[clÑ¿æö&Ó±öæ¿àK!2߄UNASNonenone%?¸a6ŸÏ/9?¬
ã)øÏ?ìóÙ,?¬
ã)øÏ?áJÈæ'!+?ÔsN\g'ç?Ýjn3±½¨?ÔsN\g'ç?Ù?‰ç
®?¾,®|ù?ã`;yt©?¾,®|ù?éMUK3š®?ÃéÿÔ/n]?ÊʪÓ1•E?ÃéÿÔ/n]3FGL J1901.5-0126@@f…ÂL@JÀ]Ç@›Ñ'À8	ð1UãaÀ:'%ž:X?ÝÜ背'ô@fÖ
hHi@ò'ÿ¿âül`(‡¿èõÐF~êl¿æ"&Bý"¿é¢ó*ë¢6UNASNonenone?黕;8Ñb?Ė'ô??É«ºz?Ė'ô??äý°Ç1;N?Ñzª+(£ä?Öžq‰f?Ñzª+(£ä?ä2vI½z‹?¸Þ׸µ?כl…
é?¸Þ׸µ?è<Y|ñ×ó?¶ ¢ÚqR?Ïš8 5?¶ ¢ÚqR3FGL J1902.3-3702c@v~ᛐëÀ1öwÄ\»ÃÀ9¾'²˝À;]Öì
¶?òb̓ìÜ@
ÈpëÐs @ˆ/ž‹q?ãÕG§€ÚR¿æ½@šF_,¿ç¾™è7Ñ¿ï ÖÊÛ
¶UNASNonenone ?ºQ:Ç·Ë?¿‡CÊRÂn?ìµØ¿G	?¿‡CÊRÂn?Ãö`]~0Õ?ÅýÕ¨‡?ëgè sË?ÅýÕ¨‡?֌BÙ?¨Ù?¸—LêWàÎ?ä¹Þ"`+"?¸—LêWàÍ?ÀÞ¸nU	†?¤uô™æÇ?ëÈQäj½ž?¤uô™æÇ3FGL J1902.6+0655@D/Ù<FØ,?åԄƒEÀ8‰GnSš²À:Vgâ?âà:Üä‹Ê@áÊf–@؋Ÿ…ì¿?ïý—"ìпæHXT¼2¿âoO°0M¿¿å¦ÃQqUNASNonenone?֐m˜o?Ñ)P©"?ä·Éq³Èt?Ñ)P©"?ÒÈP)EF?ÒêÖi$?æ›×¸k]]?ÒêÖi$?àÏã/φ~?¹'˜×H›°?Þ`9 `ó?¹'˜×H›°?ߣ`ùOO?Æüäàcê?à.OƒXX8?Æüäàcê3FGL J1903.9+0052@A'ʽf'À*ï9ßßÀ9O²G^cÀ:‡Ð|"µÝÀÙchÛ
Ó@ˆí$C@'& {±¿åšxBB+¿ïÇ>㕑!?í<F'Ej¿ãÔl~XuUNASNonenone?ï¸×ô±%?‡bšäñ?Êܓ¶£?‡bšäñ?ï`˜¡¿?®/˜SN?"ìëÈ=Ë?®/˜SN?í/"«?§ÉbÀ¶!…?·Žƒßú£?§ÉbÀ¶!…?ïÿÿ@>À úkÔõØ>‹ïû¾V+Ç>À úkÔð3FGL J1904.7-0708@<>iƒQÀÒWBÜôbÀ8'
DŒ!À:ä
ƒÁ¿ý¶3@=Ä×5›@²=@RU¿èØ(Ë{>¿ã@ãëªæý¿åø|
Ë"[¿îkìï.UNASNonenone?à‡ð:¶ƒ?Ì^±3G?ÞðŠ"öø?Ì^±3G?î÷?±¦vq'6? '.r?±¦vq'6?äl hèÇ?¶f"«ÛŽ?×'Å¿..s?¶f"«ÛŽ?ï÷ŸMW'?_W®_‡ø?PÁdÅQ±?_W®_‡ó3FGL J1904.9+0818@DîE܃#6?éẃ}™À8̀eëí$À:&h!Q‰?Äw,S½d@û‰Eû7@`<`ƒxp?ìÏ7x¾ê¿î›æË{"õ¿Êï,ÀtÇ¿Ü}ìÑ
ZUNASNonenone?êC$"²%?Æ3"5½|?Ǟómí7j?Æ3"5½|?é`#Hð?Òج¸œ?ʯrßøD?Òج¸œ?èÞ.PL?²Ø]ҙ"5?̇ÂF¾Ð?²Ø]ҙ"5?ïÇÿö'Á#?ƒ'RM‹´g?|¶Ÿná?ƒ'RM‹´i3FGL J1908.9+1022@F©æî·?ìJ¬áõÓ×À8T=ÚV"LÀ:1@\¢?óÒ‰šs@
£'䞥@®Ñ¾¿â^ñ¥™Ø¿ç©Õ7Ä+W¿ëΐÌEò¿ßº¶L5kUNASNonenone?šž³´L?¯/F²?ï+
b_E ?¯/F²?Ðê0é	}?Ð`˜gô¾å?çý
ç‹{B?Ð`˜gô¾æ?Ò͒ÿ$0?ºøIéYê&?æ™6€mçþ?ºøIéYê%?ˇÜ~"­m?¿¨•·k‹ï?éàZÔ¦?¿¨•·k‹ï3FGL J1911.1-5318@u{sBí»ZÀ8Jt֐›À:&ÇÚÄçÀ;¼¦Ô¿«?óŽP:U~@
hÍ°LŽy@žÙ€\¿Ó3T·xì¿èx1Ÿ+Ì.¿î~.ÔÝ¿ïþEõF'_UNASNonenone?Þ¸–tRf1?Ñ;Ñg±¼í?ࣴÅÖÌç?Ñ;Ñg±¼í?Ã6M2Úiò?ÆûÊA®?ë2l³Ieƒ?ÆûÊA®?à"ƒ,
>?¶^å»e?ß»Úù§åƒ?¶^å»e?¬ë•ÓœNù?šòŽÜnu{?î1F¢Æ;?šòŽÜnuz3FGL J1911.7+0307@Cº`Àœ~VG4À8ö}«ýIlÀ:·Ÿíp±¿ùMÛÅãúf@Á~Ëb@"éßW=ÿ¿å&5Bpם¿êE[–¿Úx+¸ô~¿äùõ§ÓUNASNonenone?ïäuàÅ¨?rÜ׈BzÂ?kŠp:XJ?rÜ׈BzÀ?ïqP
"e?³>UÑtKk?œ'Õþ­s`?³>UÑtKk?íY绸1?§\ç×!)?·0Â">w?§\ç×!)?ïÿ0Çh¸ü?&A±/f´?çèàˆ^?&A±/f´3FGL J1912.7+4610@SJ«Š\å´@/‹ºw_²îÀ:>´~!nÀ;Öq»g¿áŸoã×o,@.ÁÕøÅy@‰àiÝ¿è#ðÿ㭞YzxJ¿äf¨6{£K¿åðËLD&KUNASNonenone?ïíMMµT?ehБaìí?b²ø²J¬}?ehБaìí?ï¹^®t?Š¾}«$?¹¨X"c
?Š¾}«%?ï)­üzÀL?'å;aAÂ?šÊ@p§ö}?'å;aAÂ?ï¹î@ZyÃ?xßbÇ»ÓX?"oéaJ?xßbÇ»ÓX3FGL J1917.1-3024@4¹£$\×À2x/øìˆÀ9MG8£µÀ;d¿1ٖà¿íž÷ì$Õ@¤[«Ltx@å6ÿñga¿çù@Éì¿âÎSEÞlÄ¿Þß4½eÀh¿ä$×3"=UNASNonenone?ïãsoóg?mè«ð¦ ^?lŒ˜ñ¦?mè«ð¦ \?ïÃêmøW$?‡qöǚ?~
ÉÔn!?‡qöǛ?îÐ⋀©Ÿ?—iLàY?¢ñ×Gõf?—iLàY?ïðâg]pº?[¡ˆF›
?^;1E‹?[¡ˆF›3FGL J1919.0+0452@D76z—À¡±–¡À9!çû&|lÀ:½;ÇVkG¿ÆUm*QQ@2ÁÇ`&@Å'ßÂó°¿á•·*ã¿îIîª(nD¿Éy_+Mz¿åIĸ3ìUNASNonenone?ïZCجŸ?Ÿ¬Ë²Ãœ{?"·"êlÓ?Ÿ¬Ë²Ãœ{?î׫Ȑåƒ?±L^?xª?¢…Cvñ§ã?±L^?xª?ìP"ã(w?­
†U8?½{Xæ¼Gq?­
†U8?ï¶B}8Á?ƒ•pIrä?'o|à±Ïö?ƒ•pIrã3FGL J1921.6+1934@JÝdob@'T¡B‡À9,¶5±'µÀ:©-Ú-Þ?ß6ðôfÞ@
òA›«Â'@òÛ¿®×¿ã)¯–Á¿èÚZ~%Ë¿åw‹Dl@›¿ìÌx('2ìUNASNonenone?Ë?cNæpc?Êlw?Àk?é0',Fcç?Êlw?Àk?ârå@'25?Òɟ°æ?Û5±›–?Òɟ°æ?ád¦6LD?½@â`4Î?Ý6³"gïy?½@â`4Î?ãÂÎ؈¾?Á'èüÑ?ÙÔzbNî?Á'èüÑ3FGL J1922.2+2313@L'Õ'å!W@B™ØƒºÀ:CĆ­-ËÀ;nÏM°Œû?Ý[ò¤ÍªB@4˜³•™/?ùÿTžè¸ç?ácØl"&8¿ìl‰‰3Îl?åD\Ñ<H0¿ºhkÎUNASNonenone?ïý)¸ƒÌ?6ç•}瘮?6²?ûá á?6ç•}ç˜Â?ï¸íš!`/?—;ˆãÙ¶?Ä™w§ô?—;ˆãÙ·?ï T›7­>?ƒJîm=?‡êÙ2°L?ƒJîm=Ÿ?ïý(ºI:¶?M5›±‹®ð?6º-¶*L¡?M5›±‹®ý3FGL J1923.2-7452@sÿ'}keªÀ</Ý÷vÅÀ9ŽŒŸ5À;ª­œ…Ý$?Ûs!ëb90@mdÆ~)&@¿¥`w9¿äh1à«Y"¿æå"Ód—¿ÚƒKÀY>¿â®xŒ6bEUNASNonenone?ïü]ÃI¯d?BNo3TÀè?=岄ÞT?BNo3TÀð?ïÅÕ Y5Þ?…cÛÂYî?}/Óe?…cÛÂYï?ï¢~•ð[?‡ÅɇÎ?‡`Zƒúi/?‡ÅɇÎ?îëɨåH´?‹¾ü¿Ú«?¡Ceq«tÈ?‹¾ü¿Úª3FGL J1924.8-1034@;("ƒ‡ß]À(V*€JÀ9ÓôzùÀ;7›~v'¥?«x¥"éœ,@™Ã
+R@¾¦ ™@¿æ'H"¬:¿åÆ#aÃ¿Þ¾ø+}æ¿îÁç«lÍ*UNASNonenone?çóƒžtÊ?È•2¨ñÖ?ÐøÃæm?È•2¨ñÖ?éITç?˃þŽI‡ˆ?Ëöۓº¬`?˃þŽI‡ˆ?æ vÀùÒ)?º%v~Jo®?Ó¿~[­?º%v~Jo®?ìoçCJw?°P·Ò?9ì?¼€Çuå¬P?°P·Ò?9ë3FGL J1925.4+1605@IŠ3:}ª?zíݵõ'5À8	êâa‰ˆÀ:,îÉvÖ÷?™çÿûoÅ@µ…7âÅ]@À ý¿âî‹ÊŠ9¿é&¨¨L²-¿çM=«mh¿Ýü3¸ûDëUNASNonenone?ÓGäD:év?Ï@𠡖?æ\
Ýâ‹E?Ï@𠡖?Þe6}u³z?Õ";çü?àÍdÁE&D?Õ";çü?ߒv¤›ô?º"'g¸4?à6öD­²?º"'g¸4?ëp³ôò>ž?ºáSÓïµ?Â=0,7‰?ºáSÓïµ3FGL J1925.8-7826@s¾ó¶E¡ËÀ<@ýâïNÀ9¢îš|îhÀ;m溴œT¿´[jƬQ@
¯G·Ï @`aꁿê4,s,À¿äøã5U€¿á–"ö¶;¿ïÿÞ$8 UNASNonenone?ïÒT1ò$\?†ND9ðR?vÕçíÒ?†ND9ðR?í=N"õÀÅ?¼Œ%5‡‰€?¶ŽèQùÛ?¼Œ%5‡‰?ìÄæ~H	Ù?§MYZÒã?¹ØÌ
¿±5?§MYZÒã?ìʧÇí³?«é¸Á;fÚ?¹ªÇÁÀ'd?«é¸Á;fÚ3FGL J1928.4+1838@JÓý`éNä?âz
w·Ç'À8‹iŽ9GÀ::
fðÏá?Ղë݉2™@
ÖLØ À@S%?ªá?âPîû¿èŸÛð¿è³ü"±E¿Ü3?_2âÎUNASNonenone?·8¬Øx<?Ä2~mÒÐ?íêdðø}?Ä2~mÒÐ?ãEÖÅ$?Õ&€ÕZº?Ù÷tRu·ð?Õ&€ÕZº?ß;œ¢þd?¹~ÏI Æ?àb1®€ôN?¹~ÏI Æ?êºå»Bª?»‹¥³/A?ÅkáõV?»‹¥³/A3FGL J1931.1+1659@JBeÛ
Ø¿è…uŠÆ—ÿÀ8›Âª4À:DÏkã}é?õekÒa^@žûo! å@üN¿ÓÀ?ßðÉæ,^¿ãÌjoEĿ麃㾛¿ïÿA¡DUNASNonenone	?i[Ñ\9g?¨Ù{yÊ?ïæ¤.£Æà?¨Ù{yË?"ÑLBìA?—¸õ–Qh?ךּ͊ôO?—¸õ–Qh?¦u\Œ¯›?Y¹N5J-?75P?Y¹N5J/?¶¥O,žøM?¥Rå_olT?í+Vl ö?¥Rå_olT3FGL J1934.2+6002@Vôå´$_[@27Mœk2À:Uî²ÑÀ;ö-±l¿Â†J~˯c@˜zãKz@nÿg(Ù¿ë³e"®£¿ÊlLJE^¿âð´ÁúG¿äKR6·)ÖUNASNonenone?ïÈ
†³Ç?†ôi9¦PÍ?{òù<¦¦?†ôi9¦PÍ?î¼j?J¬t?­šºŒ~œ?¤9\U8É?­šºŒ~œ?ïZ~ßÿ|J?êVVà¦?"°$vÁ?êVVà¤?í×E¤ó˜ù?¤Ó¼ï¾É?±EÒØc88?¤Ó¼ï¾É3FGL J1935.2-7924c@s¬Ç£˜ À<£IàâiÀ9z¹9r•À;J›'§å?ä1äèç#@€9'ù@|#ꬿÇI(]ANª¿íOŒ³é7M¿ãÒìa›."¿Þ$Tý¢UNASNonenone1?ïÍúÝ.P?€ß¥fWg?yõhØ?€ß¥fWg?ï¼­Km?×4díÅ?€ø¹-$Ó?×4díÆ?ì‡"û[?ªà@t»?»ÆïÀ'…#?ªà@t»?íB7κM´?£ÄËGÞ8?µîAŠ-'^?£ÄËGÞ73FGL J1936.6-4215@vJ¡BoçÀ9Õõ'^éšÀ::7yéÑÀ;³¢/jP×?ðº<|]@ò¨ À€@w)¿ìêz¿à
TYôh¿Õ¬¿;>Åc¿ê¦;Ë`ˆ¿ïÿ…'yåtUNASNonenone?×øK>mçL?Î2•èGgµ?äÚ`ÉZ?Î2•èGgµ?³±û"Å?¸rÂ*Øî?흉Þà›¨?¸rÂ*Øî?ÞùtGí‡=?º'Ä"?àƒEÜ	<a?º'Ä"?³lÖº©ëœ?™¯bWPR?í'e(ªÂ?™¯bWPR3FGL J1943.8+2518@NœwškP±?殧]Q"ÈÀ8ÑøAÆÀ:œÁ>#Q¿Ï…·3@
›WœŸ˜@Ó0?ß|¿ß	-#,]Š¿èwu[»e¿æN¶¶#׺¿ä‹oVÇYUNASNonenone	?âÜc/¨¾?Ï2$ª"Ø?ÛòG9 ®ƒ?Ï2$ª"Ø?åž‡€Ç?Ôö|27¿?ÕæÂñÌþq?Ôö|27¿?å•–]ø?º^'ý˜(Ø?ÕÌÔÓóD?º^'ý˜(Ø?îˆÝD@_¤?¢ ђ1Ë?§r+»ú¶?¢ ђ1Ë3FGL J1944.0-0535@@óò^VÍlÀ,u\WìÀ9ðáù"»¼À;D"uuÍâ?К"»Dua@|Eëòè@ijàֆ¿æגMŸð÷¿ìð¯fEÀ¿æI8̶b¹?ÝڜÝàŠUNASNonenone?ïåi¶¯A?s*K¬ä[?j–IPoÀA?s*K¬ä\?ïÍҘ¨æ?‡Ó ^§eM?y³«Œü¾?‡Ó ^§eN?ž_?š†<<‡ }?¤'f°?š†<<‡ }?ïò"—äeK?aÜ]…D)?ZöÐ75j{?aÜ]…D'3FGL J1944.1+3919@R^ÞÁÁÖÐ@V:ADmîÀ9Ý|š…RÀ;€½I¢¿Ã‹
¯ëëv@
,"GÓ@yğ»¿àôõG6¬¿ám5Ù¼Ûy¿ãä$3¢*¿æn`I°'òUNASNonenone?ï¸ü:°Ÿ‹?Š)ëÿÏ Æ?ÀñSØ?Š)ëÿÏ Æ?ï›hT¸‰3?˜³õ	U0?‰%êÑݳ6?˜³õ	U0?ï$ÖëÒA—?"4Ž™Çœ?›e"…·Í1?"4Ž™Ç›?ï—da2µ?~…'A·>5?Š&ù'³RË?~…'A·>43FGL J1944.8+4300@S3¦µ(@"{¶NGÀ:Z©D1ˆ8À;¯¾ÌY	‡?ěáµ­E@
uËc–'t@!¿ím?ïæ"GÂP6¿Õ{è7È¿Öü}ù™Î¿æ̟m™
¨UNASNonenone?ïé䳏?iÎÙv+òÿ?føLpý
?iÎÙv+òý?ïW¬üz°?¢qÛ吞?•
`pª?¢qÛ吞?ïGƒåà8?A½;¸H?—ƒCøþ%?A½;¸H?îÿÚA²F?'"`÷*OO? "[äÛ ?'"`÷*ON3FGL J1945.3+7329@Zd¾ß¤@@68üPHðÀ:4i¼\<AÀ;µò×s?ð9»þHoÛ@þ@ô'âÁ@XY …F%¿á1ÆT˿룠ÞÝE–¿âÔSÝUd¿ïÿ™`Â@5UNASNonenone?ï'åæ¯ø?›f'}"?F¸ÆT
?›f'}!?áL›-N?Ð|Ó«cøN?ÝfÉï¥ßf?Ð|Ó«cøN?é7u)š?²Èì
)Z?˧"+ÓYœ?²Èì
)[?ÏccsX?¶(úö©ü?è''#)û?¶(úö©ü3FGL J1947.4-1121@<æÀ§¨À1'äy'¼À9À=h@[:À;coF߸b?ò¼¥¸5ç@
Ê8ƒW
@9T h«:¿áã¼üS¬¿æ[Ëû
¿ãàý·©ê¿ïÿÆòmESUNASNonenone?Þä
Äy?ÐՑ.²}?àùÃpÁ?ÐՑ.²~?ɬtf´—´?Ên!™)?é"âæRÚ?Ên!™)?àA"¡˯?¶u53+œÂ?ß|ö½Àh¤?¶u53+œÂ?Âô0m6RV?«š,Oß?ëBóä²kj?«š,Oß3FGL J1947.9-0743@@0,ÂÖ©ÅÀ0"ý*bªÀ9›A<á1ßÀ;WæáK	?ä]š@ÀgŽ¯…¿@= ˜ò¿ÅfÈ/¿éԇõ¾nÌ¿àiFî?Ó¿ïÿàí¸w"UNASNonenone?ï͍"e1;?"Y]Í5Ã!?y95Ígb=?"Y]Í5Ã!?ì6º°¸?Áê+(Ëéu?¿'ŽJ*z??Áê+(Ëéu?ê0)Z±gY?±@Ë¡~Y?Ç?Z•:bœ?±@Ë¡~Y?éÌr¡ç7?±õ</Û?ÈÎ6xc%?±õ</Û3FGL J1948.1-7059@tE¤Ý/ À>#óYÿO×À:8	=–c"À; ±Po"¿ùë›oÉ@›-—
H@¤è¿òsпçÞтFÊG¿èÒ=؆¿áɆµwÓ¿å"DkÐï­UNASNonenone?ïýÌS¦åÄ?9
–}°ÇA?1bÈÑåœ?9
–}°ÇH?ïé΃–?pÂ>ä
AZ?fç1ë|jÿ?pÂ>ä
AY?ïrâõA?‰iÃ[,£?'¼=c¡Wï?‰iÃ[,ž?ïûôm»ƒ\?B×¾n¬UQ?@.Iò‹(?B×¾n¬UE3FGL J1949.5-1454@9¶¹ä'¼0À3v…3±tÀ9´ÒŠ{ïeÀ;n"WBÜô?óZ¥óš@s¯H'zÄ@Ž@À9–z?ç=Û­»:¿åJÁI-gå¿ægò(b0¿ïÿωþœUNASNonenone?âZsf«è?Ò$!ÈÓr?ÛJý2¨.?Ò$!ÈÓr?Ö%á¸+ïµ?Уæ«r«O?äí#ê&?Уæ«r«N?ÓÌÐUñW??¸(z›;Ÿ0?æ—ÕT`?¸(z›;Ÿ0?Ñú¸×J‰œ?´t'Ç3-?ç£"Z»2?´t'Ç3-3FGL J1949.6+2355@NXG¡A)¿ñ×Ê÷àvÎÀ9#ª¥æ¯À:€Ú†?à2»œ"àÖ@7í&ßgÚ@Z¶ 8Ò¿Ü·N´ ·
¿Ö³'|¼6¿ì"žZ@	Ó¿ß21k

UNASNonenone?ś½RT3H?ÊC³-1Û?ꙫjó.?ÊC³-1Û?ÐÞ$Š¸Ñò?Ð|àvÊ6ƒ?çíº£—?Ð|àvÊ6ƒ?ßÄ1½P3?¿Ô_0´?àç!W¿e?¿Ô_0³?ÛÇëOˆš?ÄIB G‹e?â
X;²ô?ÄIB G‹f3FGL J1949.7-8109@s‹ohÜÀ=ãæÄŗÀ9ÁC
›ÉöÀ;m±|å-í?ä¢X —>@VŠ16"@šwàŒGL¿Î"tŸA×Ŀ飨Dhuñ¿Ø©Ý ¿ê®iÆ~eUNASNonenone?ïõ–	~ÏÃ?_•H~½r?TÓí`z¸?_•H~½t?ïÄ¿l<2?†¸€<‹˜d?} IáæôŽ?†¸€<‹˜c?ìù˜eƒ«??¦—. -¼?¸3<Óâ¦?¦—. -»?î~	XÿF˜?•¦ÔK†E?¨jp–?•¦ÔK†E3FGL J1950.2+1215@IS6Þ¹^[ÀxK èBtÀ8Ù°i¿·;À;øìˆ3?õ…*ôö6©@Q¨ò'$\@à`}n¿ã
l"Y¿ç¨6©EšO¿í‰Îtäûº¿ïþfå^¶fUNASNonenone?ÅÚ†ìŽï?Æ/¹±
?ê‰DÜD?Æ/¹±
?œÜ½6?ï?¯/Öèu­?ïO¦?¯/Öèu­?×DõÜ`»?¹Læ1úÂØ?ä]…ϸ#?¹Læ1úÂØ?©ßX…¥È?—}†)´	i?îb
w¥£?—}†)´	i3FGL J1951.3+6909@Y]uÍ·@4#ãŸw),À9÷Š1FÉéÀ;À´4O'å?Ôîhæ¦ñ@Òbœ­JQ@•ÀoF_¿éí$
Ú¿ëÒÑøß¿åْ 1+z¿Ý.ÚáÆUNASNonenone?ïúqŒ°gù?GêŠa:ñ‡?F9Í>`"?GêŠa:ñŠ?ïÓöó¹?—ÐL%æ¾E?‹ËC;Q"?—ÐL%æ¾E?ïsÁv"ñË?‹
É5rU@?'‡Ñ;¡Æ"?‹
É5rU=?V˜jü?˜3éåü.(?¦ʖyP??˜3éåü.(3FGL J1951.8-1102@=°É2
™FÀ2[Õº²À:Á!ßyÀ;eºßd?èr˜7]©@Ûï«ÉòÓ@֓À;ÄÒ?ï_»eàô;¿Üѳ¼©¿äÆ«¦j%¿Ûy%è"JóUNASNonenone?î¾ÄðbÎ?ª+ˆ2.ŠŸ?¤S°ùÓ?ª+ˆ2.ŠŸ?î¬zØI?¶8ø'«¯'?¥>ØW{y?¶8ø'«¯'?ìqgš´?­Ñͳ?¼s|Ç3*^?­Ñͳ?é58G¾5b?·J?­ÏçC?Ë+á*w?·J?­ÏçC3FGL J1953.3+3847@RzAc
'@~¡ÆÀ9T†È½¯À;
»3GU)?êU7°×‰û@
ë×j@zoÜÝ¿ÜòD…ëçÅ¿çÜ%ìèdó¿èz0¶èE4¿ïÿ™àóUNASNonenone?ã½£}»÷v?ÎÒ}¬qËc?؄¹ˆ?ÎÒ}¬qËc?ÔÐÿT–#&?ÑïùâÛ?嗀U´îm?ÑïùâÛ?âãIäfÕË?¹'{V?Ú9l72Tj?¹'{V?ÄÌ<
!8?¨VO‰~VZ?êÌðü·±ü?¨VO‰~VZ3FGL J1953.4+7653@[LлnÖw@6ö¦ڜ™À:;[dRÀ;Èp0ꃗ¿Ð1¬¦ÍÅ×@¸1Hwh@ØÀ€
V¿å>ú߄µ\¿èUDÔxñ¿åCŸjþ&¿ÝÝ=ÄUNASNonenone?ïø$,w?R¢«H0 ?O¿¿oN$?R¢«H0)?ïÎDkÞ?o@Ñþ?xÝÿJyÝ?o@Ñþ?ïjwT´a?ŽÓÁ¯lŠ?'±isÝ$?ŽÓÁ¯l‰?ïÒF½¾¢;?pMpÂâŒ?vÜ¡ ®â??pMpÂâ3FGL J1955.7-7019@tQ!–R½À>ÓKµáÀ:p‹¨?NÊÀ;̽M#Ÿ?Æì,­Nœ@
+Š•š±@
@/p¿ãã…³¼8¿Ød™ó‡¿â1|ÇX¿á£LúôAJUNASNonenone?ïú,ñ1Ë?Kâ~˜Ï‡×?GL;÷8Փ?Kâ~˜Ï‡Ñ?ïËyý?s?"ÉV\ÇÆ?z}C`FÓ?"ÉV\ÇÆ?ïtýøÿ…_?Š7Ú#0?'`@àT?Š7Ú#0?îÌÈýß4á?°zu÷ô?£3p"±ú?°zu÷ó3FGL J1957.9-0712@@ÿùÆ*\À2Ò^Ý)À9ÊØ>À;rȖg"¿Ð¼[\ê^%@
£prƒÖ@Åz¤6¿ã
e'ª6ö¿éÓb¾™¶Ó¿á"3©®BQ¿è‹Ãÿ/UNASNonenone?ï̋†l03?'á'³¼?yº<Éçæ?'á'³¼?ï1a¦pP?¦ß·Aóíí?™ÓßË1ö?¦ß·Aóíí?îúΚ?–ã"-ïŽ? ^Ž~Cp?–ã"-ïŽ?ï'QìC±?'S°LTt?
ÕÂw‰ä?'S°LTt3FGL J1958.1+2436@O#´·,ÀQ½í@À9Õµ•x¢©À;[L
ÀÛ¡šÀ`@Ù2¹e¼È?úÜjŸ01v?æM"xºžC¿àƔR̚g¿³4ÊþҔž¿ÛPý~"xUNASNonenone?ï÷x³Ze?PÐAð‡V?Q™K5ü¬?PÐAð‡]?ïKÐrzeº?°s$|?–…ñ°³H¶?°s$|?MyA?…=Úig'Å?‹X졯¸Š?…=Úig'Ä?ïÿþn0p¤>Áå
a0«z>©øõ¸e>Áå
a0³i3FGL J1958.1-0243@CЀ¶sÅÀ0>h›À9‹•¢"À;Vé<o?ÇÂyë1@
O^b@ìi_À¿à—%oŒ·¿êðò	áð¿è9/B[M¿ïÿ®7¥!§UNASNonenone?ïg5<õ'q?¿¸"Ê,Å?"XaO±ç?¿¸"Ê,Å?é=¾âÅN?Ëøî9Jõ?Ë	w¤êÇ?Ëøî9Jô?êÛ^À?­™ vù ?Ē‡©¼ýþ?­™ vù"?èA§\Xœ?µº¸,"u]?ÎùbŽž"?µº¸,"u]3FGL J1958.2-1413@;LŽÞT´À5§ÞÖºŒÀ9Õ¤9/ÌvÀ;t_˜?õ#¡Å¸@Ä
Ò¦€ˆ@Q%¿'6|¿ÀÈk%^¿ê!ÁduÍ¿íi=®ŒDò¿¨ÃG.ÇUNASNonenone?Ù%Þœ9Q?Òb®Ûü']?ãmÀ1ãW?Òb®Ûü']?êéõÅ?ÒcÔô'?ÇÌX(뇼?ÒcÔô'?äì}»ÏU?¶ÄÖÅöµ?Ö'ˆaUð?¶ÄÖÅöµ?ÔÕU#—£?̜Oo?å•Un4~/?̜Oo3FGL J1958.6+3844@R™é9êÝY@hg~"Z•À9XÓÍ$áÀ:ﺽ֏Ä?ÚlƒÁH¾@ÉQàd)@PŸGƒ¿é×*'EÑ,¿èZAâÎkÞ¿åþ	WŽÿ"¿ì+€áUNASNonenone?ïdâ·ºÁÕ?šÆ+'[áº?"c©§ÅI?šÆ+'[áº?ïKú*Ô(ˆ?§ig™|8j?–€º¥zï?§ig™|8j?ì÷°œèè%?©°À},?¸B{¸¾à?©°À},Ž?îD¬—¿ÈŽ?š`y#³h?«µ6"w?š`y#³g3FGL J2004.4+3338@Qªõs}¦?ò÷; ¿þˆÀ7Þ@c^JÀ:›ò¼K?óp"£¶S@WÉy[5±@^Ø_ýì¿àáÐûø¿æ]ª8*òP¿äË4àÝP¿åiÀBеUNASNonenone?¾Âª5}'º?½üêoΐÊ?ì'ª¹PMÉ?½üêoΐÊ?£øœWp¡ï?·Ö鏾dD?îÀv:ˆõá?·Ö鏾dD?ØW;81XË?¹R~Ýq†?ãÔbcçS›?¹R~Ýq†?ÃE±òÀ§7?¨_èÖ¦?ë."ƒOÖ2?¨_èÖ¦3FGL J2005.7-8241@smÝ/Ÿ¾À=:úÖËSPÀ9ë:жfYÀ;‰$Ų&?Ï­¥EýÄ@ُöÏc@p0`E)¿ç"A¢¿é¶ÔÕ|@:¿â»|y(¿ïÿ­½Æ}0UNASNonenone?ïÿÆÇ95?b¶-B>üœpãe# ?b¶-?ﮅƹ#á?"éMi–<?"^ŽQ·‰?"éMi–<?Ki3?"]Û a›L?‡Z|-%³t?"]Û a›M?îוW¹ ×?"ɹy1]]?¢†ª"mò"?"ɹy1]]3FGL J2006.5-0939@@Q'>EÀ5‹&9O­À:˜._ŽÜÀ;¥1}PŽ?ï™ÿ¤ª2³@õæÌ}G@~Ûÿo·H¿ÜBÈÍ
åF¿éC¥×?—p¿ïþOÃ%ã?ïͦ¦óIcUNASNonenone?îíë$9pÁ?©ÈFEÏì?¡!M¼hóõ?©ÈFEÏì?ïp¬…ÕÉ?°pêb^?'êoEFÞ?°pêb^?é›2FHs?²Bªª¡§?ɓ6æÞ3ú?²Bªª¡§?î¾ßf2?¸	øk?®Ô	žlà?¸	øk3FGL J2006.6+0150@E¸²•éá±À/aǛ4¤À:3ùJYQÀ;›zé¯?ðÝ ,e@:%Ïrn‡?ýô€kJQ¿ãÉÁb"ü?ïÍØWiJ¿á`pX
a¿çµ>LòUNASNonenone?컞-÷jm?»Ctc‰X÷?º#D¬˜?»Ctc‰X÷?ÀGIâm;ò?ȔÓP$>H?ëî-‡d±?ȔÓP$>G?èç­6þ"ò?´ËÒ7<m?ÌaK$t7?´ËÒ7<m?Ê:7ýè9v?ºèj|ò?éqr…ñ£?ºèj|ò3FGL J2009.2-1458@;³íÇïzÀ7Ôé8yÄÀ9¢eYöì[À;d¸€åm®?ñK×+Ë_å@i›ô<ÓE@' ¦Ô¿å|!SŒÄõ¿ë¹©#Ð>Ç¿éŠp|h¿î¨#§Ù›UNASNonenone?×øˆ­GþÑ?ΦÈ(
¹"?仩\˜?ΦÈ(
¹"?Ë=™5ì?Ì8HĄ_Ê?é?p™²¼F?Ì8HĄ_É?ãˆ][¸³7?·D¸w»x?ØïEHŽ™'?·D¸w»x?¯†E_Êp?š¬ˆ>Eù?î›®:X?š¬ˆ>Eù3FGL J2010.0-2120@5Fw_²íþÀ:f	EùßUÀ:.P‹2ΉÀ;¤#ìnS?ñŠ¢`<«­@
[ûÈ7ç£@l€xá=?ïü[J ¿¹i8þ6AÕ¿àÊÂè-·"¿ì¿.Äí
UNASNonenone?LJ˜âôX?ÆáQ$&Š‹?êÇBܪ?ÆáQ$&Š‹?Ӝ@Š?ÏܵÆW®?æ1ß÷rºð?ÏܵÆW®?Ðe]ÍZQ?º×ây_:?çÍQR×|?º×ây_:?ÒŒ×uDú?¸£÷ÿj–?æþ9"E]ƒ?¸£÷ÿj–3FGL J2011.1+4203@SŸ …±…I@_î} ½À9?Ú{9À:ÈTà,%"?õa
1@ë@
²ká$ž@I« §U¿æŽXõÜÝÞ¿ê÷å#¿æøá–ïi¿ÝÃëfjUNASNonenone?ç£Í(!?̱ýa³9z?ÑÒ¸e¯ç¾?̱ýa³9z?ê.¼×eÐ?Ñ!üSu¨_?ÇE¢h¿æ?Ñ!üSu¨_?åS®Ë'[Ú?µX^C³'Ó?ÕX¢hÛHL?µX^C³'Ó?ÑP…"^"?ÀðrɊc+?çW½=þж?ÀðrɊc+3FGL J2014.5+5246@Uøígwž@#Ìó˜éprÀ:3o­7PÀ;k¹Ù&w?íRŒ#†º;@#¶XzÀ@bÿèƒ¿éõ'–âd¿ïÿžæWê?ïúu7B?¿Üº ÆUNASNonenone?ïýùí@ü?5^î÷ìR?00•ø\=?5^î÷ìO?ﺟ?•œ¨?'»qf–õa?X0˜Ö;?'»qf–õa?î²®+fR?˜5½•ß±æ?¤Õ½Išé?˜5½•ß±ç?ïÜS^æD?–¨9íž'?qÖPŒÝ¿?–¨9íž&3FGL J2015.3-1431@<ÎdÜY2À9oç¨mÀ:­{έxÀ;µ}Ëùï?ÊÈ­Ì_N@úٝj´?üSQ@g<?Æ]E¶©•?Èk"…þŠ¿Þ{V¦-¿ 2
W!<UNASNonenone?ïÔ˜ÖíQ?~a‡rb<1?uÿ3"‰WE?~a‡rb<2?ï×Ãtam®?€¡îá3?tEÏI(æ?€¡îá3?ï!|É´"D?'X)n…8?›ÐfÉm—{?'X)n…7?ïˆÕO5j?…¤
œr?Ê¬<r¥??…¤
œr3FGL J2018.6+4213@SÙÆ*\}@>"ՔÀ8wöº «À:€
è j?ñŽÑä›@¨RÙÛ_@&«ÿÍ«¿Í¡Bt2œ¿ëAlKO+.¿ÜáÑÁŠú¿ì
2ŽÈìUNASNonenone?›ßÌúvøB?£»ÿŸ(Ä?ï!˜,H=?£»ÿŸ(Ä?¿Ž¢™(l¾?ÅAŸÀê*F?ì+¬Úòh?ÅAŸÀê*F?Îì9›" æ?´]é¼Ær¦?èDñ™×Æ?´]é¼Ær¦?¾º^$Žá
?¬·
²9#Ÿ?ì(´;n#ß?¬·
²9#Ÿ3FGL J2022.2-7220@t%VÿÁßÀ@LOô4ãÀ:¨t"ÅÀ<ÖÝÇÆÔ?ñ®hk#d‰@
>§3á?ÿ0Ñ@úÇ?䶄OÊ1?Á¿œS™k]?Ö(f")_l¿ìÞß}Ú UNASNonenone?Áa QµÝD?Ç"g¡ÛJ?맗뒈¯?Ç"g¡ÛJœ?çcSú÷«?Ôá±Îr?Ñ9X
Ä«?Ôá±Îr?Ùò·¿¯X%?¸¾÷tcÀ?㤠(Sî?¸¾÷tc¿?êüa°ÿà?Äù]
M?Ä
Ây<?Äù]
M3FGL J2024.6+0309@Gzš€If{À3%oü^À9ûUê`oÀ;€.ÓR"?ëhSÃ÷f(@"ŠÝ"T?þŸ`A^D?âa6FÒ¿Ó}Ìyjп×ÛÞéëý¦¿ì¦˜	UNASNonenone?àÝ
Ÿjþ1?Ìê|þ.«8?ÞEäÁ*ž?Ìê|þ.«8?ê4q½i,<?Éâ#jŸTQ?Ç.9
[O?Éâ#jŸTQ?â ?Õi^ï?¸CԾэ?Ú¿€U-B#?¸CԾэ?èKƒ‹FÇ?·®¡sÆ÷?ÎӉñÒäã?·®¡sÆ÷3FGL J2024.8-2331@4=Ž§ÎÃÀ>\ÜY1ÊÀ:'ý«'é¢À;̝{¦iŒ?é;H›¹|@
ßþWß:?ÿ2¼À»Ÿ?ïø̵O؅?ÚQY1¨!¿ÑçD6"¿ëŒÇÓá
"UNASNonenone?í¢`;ðù?ºaÒ
ì/?²ìþ x7=?ºaÒ
ì/?è¸6~5",?Îé(?6Î%?Í&+wO?Îé(?6Î%?èÉäÈ)–%?³wâ²eß?ÌØlßY§m?³wâ²eà?èŒFOW"?»m´Ÿ¢îi?ÍÏÂæ¡°?»m´Ÿ¢îi3FGL J2025.1-2858@,Y'fw-^À@"Ý—ö+À:TŠBäÀ;°®Xm_?ÒÓ¥ˆT½@ñ8Hñ¶@}ûŸž¿è…¶ˆ×n¿äÍD¢úÊ¿Ü?Géxª¿ÕvØiþ»UNASNonenone?ïþÊ#›¡Ç?%+W…k­¾?#]ÆEã›b?%+W…k­±?ïز¥®Õ?she˜?sö¦­(•¾?she˜?ï¼aø"M[?|Ü, 5³?€çÞì©A?|Ü, 5®?îø 	±	?'XÊÜ6ÑM? ½ÿdïe?'XÊÜ6ÑM3FGL J2026.3+1430@L¡WÞ
fñÀ*àÔº××ÃÀ9΃&À;˜(ßó?çN	÷^@ËoT¡˜@E¨@P}¿Ê/àýJ1ì¿än¸oüõ¿×û'hZK¿íi$;!GUNASNonenone?è*mÓÝn?ÅàŸÿç¦ÿ?ÏVH°ñŠJ?ÅàŸÿç¦ÿ?ê·fe$cá?Æ׃~w?Å"fknpx?Æ׃~w?湎¼{?º!Àd{·¯?Óڌãè‡
?º!Àd{·¯?êqäq‰f?±]•€S.n?Çö8n9Úd?±]•€S.n3FGL J2026.4+4709@U-Œ*EN@ÓáF×UÀ9rÀdß}©À:ùbLLà¿å|°R
 @ù|ÙŒ@|Þ 3玿â,»ç‹Y¿åƒ‹Ç·}¿í87V¯¿ '÷Ö:ߥUNASNonenone?îÐÊ-è5¶?§"œñ?¢ó]!|¤¦?§"œñ?ïÈQX†WN?'éƐ?{×S¼ÔXÅ?'éƏ?ì/ÔJNUH?°ù^ÉÓâ?¾]­U¼?°ù^ÉÓâ?ïóØÈ-m"?W "%]Q?XNo¥$׬?W "%]P3FGL J2028.5+4040c@SËà"&þ?ò[·¶»À8ÑhÉíõ<À:O¶1ÔÌ?ôù`[µ]o@š
Wǽ@р:ÍÜ¿ÒÅÈ*j{Ž¿á†qŌ‰¿ë_=ú"¿ä~÷õ·UNASNonenone4?ªK¯ã?¥Y¶ç8¼o?ïVÑC‡ü?¥Y¶ç8¼o?Éqä›2ŒI?ÍI«§Øú_?飆Ù3\î?ÍI«§Øú_?Ò1zÿ)*þ?º‰¬t¶OR?æçB€kj?º‰¬t¶OQ?É*øþS§˜?¸"u†k‡?éµAÀk?¸"u†k‡3FGL J2028.7+1012@JëÍþûôÀ0Cý?[_¢À:ˆabñgÀ;vJt˜XQÀÎރ®uÊ@ËFºÏt@ ¨?ϣ¿èº"Ÿ"€Å¿èÀží°6¿åâ'ó~¬¿Û†u¾%ȚUNASNonenone?ïÒîxqá7?§/‹ˆbÅ?vˆÃÇd ?§/‹ˆbÅ?ïÏÀsëiÑ?‡˜ÐþNÕ?xÆ
Kg?‡˜ÐþNÖ?î'ÚI9È·?šÝ—SÒQo?¦Ò[lct?šÝ—SÒQm?ïþN!_ÓÇ?6Øm]ò?+êÝ¢?6Øm]ò-3FGL J2029.5-4232@ve†á›ëÀA¾^9q;À9Ö-Š|Æ$À;±+hc–¨?îsÛïÕe@
|+Þ«¢@öã•Ò¿åæɕµ´W¿äd"p 4º¿ídÓÈÙ<¿ïþ†ìwUNASNonenone?êNZ€D?Ä×^^?ÆƗ±ùþó?Ä×^]?Аº7ƀ?ËätbD¬Ì?çü7¢äÁ?ËätbD¬Ì?çB¶i5?¶qïé†?Ñz"Ë-•Ú?¶qïé†€?Á2ͦ"!V?¬ÿ¯'ðh?ë³L–^÷ª?¬ÿ¯'ði3FGL J2030.5-1439@>Mã†Lµ»À<nš€If{À:¨ÂD³Ž7À;ÕäbÈ¿×Ûâ"Då@
h³'Š2ž?ý×>Ý
ˆ¿´SÅ)Åj¿Íºòºr,B¿àÒ­›rüf¿ØZg!ËËUNASNonenone?ïù~‹%¿º?MÒ&ú7Â?JÓiÕ?MÒ&ú7Â?ïäˆWèth?s¦µ'±?kw¨‹—"?s¦µ'±?ïHCË¥Wš?›ä %ñ?–÷†‹Uå?›ä %ñ?ïì©Ô;+Á?Y,Cìh®î?cV+ÄÔ>=?Y,Cìh®ø3FGL J2033.3+4348c@TœŒ" Ú@Ü@Þ¡À9Ý©"â À:aþ£®$?çbŽÀwª@
c¤&œ@ð»`å5?ï÷Ž›Ðù¿ë¬Î
 ©¿áÀø´îc¿ãmϟ™UNASNonenone8?í­¼×*G-?¸ý$RÍ"?²'F­Æ–?¸ý$RÍ"?êia*û—?Ì9Ö»ø´?ÆZ{çT¤?Ì9Ö»ø´?æ£4@zE‡?¸)åh‰§Q?Ò¹—tò?¸)åh‰§P?鸥ßÏØd?¿BßY"té?Éh€Àžq?¿BßY"té3FGL J2034.6-4202@vq9C¬ÅÀB0øµˆãiÀ:~L69xÀ;©Ù¿#–Þ?æ!;xjä"@
éåµüÑ¢?ÿ+žÔA
?íåÐ6c¿B¿ç&çEsý?¦®o§sE¿é"ªß½sUNASNonenone?ï뎘Ç?i&@0Wû?dqþÿg9å?i&@0Wúþ?ïXp]yÑÑ?¥
æÝÑÿ?"ñôPÅÅË?¥
æÝÑÿ?í0K?XÈ/?§Rùeɖ³?¶}¦9¾?§Rùeɖ³?îNŒ–Bj¤?ª¦õˆ`ó'?«6›ÙUÈ?ª¦õˆ`ó'3FGL J2035.6+3146@R5ËÿGs\À(IёXÀ9‡â3f^ÚÀ;Šyk%é?êTÕ£@…lP‹2Ï@fs€€C¿ë&FÌ'5¿ç¿¯æÀœp¿Ö50•ì]X¿æÓq†wuOUNASNonenone?ﮈ9…"}?äÏPM?"]ñž·`¿?äÏPM?íñKOÒ^?½¶£¹–ä?°u§
m
?½¶£¹–å?î5,%#?£PS}lA
?¬¯~]=­Ô?£PS}lA
?ïk¾o¯u?"UØovܕ?rˆ2
f?"UØovܕ3FGL J2035.8+4902@U­'#'@#M~8DÀ9Î.\3Ý}À;¨—š¼¿ê¢ä4â$@T(1ÍWŒ@Ãf?úìƿ䍙/*SÕ¿Î4Ÿ䦑¿æ¤
™¬Ë¿àˆàéiUNASNonenone?ï¯ÿvȳ?"øÁ
÷™&?""MÓ9ƒ?"øÁ
÷™'?ïÃâ·©?cø[—Ýý?~¤+põÿ?cø[—Ýþ?îAÿ.Þÿú?ŸilOî N?«à
^?ŸilOî O?ïîsÌ ½þ?a:قÍX?aŒ3ßBÃ?a:قÍU3FGL J2036.8+4234c@ThÕ¥¹c?ïèV`^åiÀ8§1"ÉÿÀ:3\m¿ <?õ"åm,©+@
êÇ+£ù@"€U$ö¿Åˆk><{±¿é={Êaô£¿æ'˦þ'¿ç
Yûsÿ+UNASNonenone9?†µë:˜¢?"¹ÅÂÁ* ?ï§Ñ(Sž?"¹ÅÂÁ* ?ÄfG,G*ä?Ér@§Z?êæn4î5H?Ér@§Z?ÓÅÉ
­ï?¸ßógHºQ?æy©	?¸ßógHºQ?ÉMn½ÎZ?¸æ"+™{y?鬤`Œj?¸æ"+™{x3FGL J2037.4+4132c@T7™E¶Ãv?ÒÙUÜ«g!À8˜-¹éÀ:2ÿâ£Î§?ê	ÑÇÞQ@
®¸–^ü@lÁÅm2?Âí'f²wÈ¿èôöЖ¿äM{‡F ¿äoñÆg"UNASNonenone ?Èy_*Ӄ?Ê |ï‹2Ý?é៨5K ?Ê |ï‹2Ü?Ö¡4SŒ?ÑÈ'R6?ä¯eÖz9ô?ÑÈ'R6?Ý_‡gÚö?»p»ÔÕrZ?áP<1L…?»p»ÔÕrZ?ãÔ2Å.?ÃÔÿK¥4?ÙÊWšuõ¢?ÃÔÿK¥43FGL J2038.8-3613@"o›™NÀB5™€o&)À9§ßV<L·À;ªÍv?ø>¿¼'ZqKØØ@
@6Tû¯ä@•P?ÞgT¿ä'@Ö½o¿ã	F? ô¿éÛIq&ù¿ä×›¡KUNASNonenone?ïå«lb?"¥ëÕ±ç®?†•$ÛçT?"¥ëÕ±ç¯?ïxðu¢Ñ¡? ÂǑ£³í?áñK¥Ëø? ÂǑ£³í?ííû¸­¥‹? ÚùcË.s?°":'Ó¦? ÚùcË.s?íäÀ‹>R ?£
òK;ò?°Ùû¦
k?£
òK;ò3FGL J2039.7+1237@L¿/˜sÿ¬À12vd
k"À:`ýŸÓo~À;®QC¿rq¿õÃ{胷…@ò…¶Æ'@Ç«_ê¡I¿æ÷쌡¿í"ccÉöP?ÔÝ!yJf¿í˜[¿Õ~³UNASNonenone?ïÙLD­ÖÏ?‡'•`?sYÝ©˜Â?‡'•`?ïÉ4%
ÐÓ?Š1`*6åå?{eíz—–j?Š1`*6åä?좐Ã#P?«ç]!¢0?ºëyæçÝ?«ç]!¢0?ïþ§˜#͘?B(Eˆ?%†}Ã&ˆÉ?B(Eˆ
ï3FGL J2042.3-5416@u{êüÎXÀBÞj㣨çÀ: jOÿò"À;¼àm"¿å±ÿ~GP@
¤ќj@lŠ I6¿â‰	Ú
¿ç"¡ì#¿éky˞¿ïû:%•»¿UNASNonenone?ïø~ô0"Ç?Pιƨ*?N/=ìæ¸?Pιƨ-?ﻂ§ýIè?BÜ̜FÉ?V­…½?BÜ̜FÊ?ïD"6?Œéµ³֍?—o|=ž™$?Œéµ³֍?ô3ò?ƒNÛUV"?‰ÖBó?CÖ?ƒNÛUV"3FGL J2043.6+0001@GNE^®âÀ8¸*º¾­OÀ:•sÔãòƒÀ;µ¤(hÔÖ?ëiG¡K·@
Ô爏Ü?ûÚ>ÐJ[?ÔSÙI:&?˜,Ɵ›˜ ?Èïx?Ï¿ãòJéÄe†UNASNonenone?ï*ˆpz'w?¡jó"U;_?š®ñð­Ñ?¡jó"U;_?ï RÌ£ì?"0ᴆî?‡ëÌ×1?"0ᴆî?î
ï.JÀö?¡Oëqˆç?¯Q
Sð¨?¡Oëqˆå?îºT>xÎy?¥~+p;{?¤Z¼sn?¥~+p;{3FGL J2043.8-4801@uúw1ÅÀC!²_c<æÀ9¢îRX'hÀ;³ Œgï?ññ[!ŽÆ@|¶M"m8@ó‰à%¢¿åŸGŒí ¿Êx=3<B{¿æVH«•p¿ïÿÜ^o³UNASNonenone?Ëü³ì´Sá?Ç3uË??éÓÒë?Ç3uË>?¦p#lªû?µp"ý÷Ȫ?î˜ýϹ5P?µp"ý÷Ȫ?ÒÜ-ÿ%(Ç?¶8…,&Ä?æ'émk?¶8…,&Ã?±÷ÛځV?L$Œ!q?íÝa"¯Õ?L$Œ!q3FGL J2044.0+1035@L)©~+VÀ32;yRÒ5À:r‰ŠWÝÀ;– f<tû?èݗÿÕQš@Fýo,Æ@S§`Ÿþ¿Æ
 œO#¿å¶ˆSåÊ¿ÙKY¥bЅ¿ïÿûC¾×ÓUNASNonenone?ïÅwË7©É?—FåïŠ?}Dd+ð?—FåïŠ?îšßÁŒ$?¸é—´Kµ?¯ÆRç=Ã?¸é—´Kµ?éñØ䘪'?³}å.ê½<?È8œmU·?³}å.ê½<?ì'þœØP¤?¬j³úL¦?»h=zÛ?¬j³úL¥3FGL J2045.6-6838@t`⡵ÇÎÀA¶Ü­¡À:kYnLÀ;¸à°¯_Ô?Äõ¿&,K@‰³*º=Ô@$¿²‡ý¿âú©/tóÙ¿ã'ú±À	£¿âê
ªþÆÅ¿ïÿóºÄ®éUNASNonenone?ïø±Ù}QŸ?VŸŸæ|?M8š
¹'Ý?VŸŸæƒ?ïÁCæV7?†ß_1;ˌ?^üTäÊ?†ß_1;ˋ?î-j®Æ? =Ó¡òh?­)^õ¨? =Ó¡òh?ï-^O|Ä\?‹1QĬ¼ž?šT6gt‹?‹1QĬ¼3FGL J2046.7-4259@vaŸ!-w2ÀCV4XÍÀ:mGÞ»ãÀ;Íw=N?(?Ö>éÜ°£@
ã͍@T kDò¿ç›s³¿×|žjÓwP¿×ƒ¤a–v¿è_¤]ö]óUNASNonenone?ïó€ò%âÒ?]ñ²U~âÍ?Xþ´:[ö?]ñ²U~âÉ?ïÎO"Ë (?€q1ëu"?xØ6oì&?€q1ëuƒ?ïDŒy,ÙD?'ÀÅÚ©Û?—npÚd×¢?'ÀÅÚ©Ú?î̹€V?"O¯=¦î?£4nnçú ?"O¯=¦î3FGL J2047.9-3119@)©IÆónøÀB°>ž¡À9Äz•ÈSÁÀ;«zl­¨D?ê…ªÉÜq@RÊ/cšÚ@*zàEûb¿êþLÂY	¿á[_Ñïó¿ã"Åãà Ð¿Ü˛Lª±"UNASNonenone?ïåŵù¿?rAÆg¶Á?j:Jü@¶?rAÆg¶Â?ï­L?[Å?—Íüö'æ?"»,ð)ð?—Íüö'æ?í¶‹ð"%|?¢Šõ::J?²K ~îÔ!?¢Šõ::J?ë--HR?±¾Qǵ5{?ëKÓJÞ¶?±¾Qǵ5{3FGL J2053.1+6027@XV'Ìö¾8@$"òsPÀ9KŽÀøƒ4À;S"9-H8¿"ø¨ÀŒ°@&§}‡ë@W§Å¬¿ä¦!'ÕbÑ¿çÃOÍ¥¿¿è_¯ðjƒ#¿ä͚ŽGgUNASNonenone	?ïÕ=‹á?}q[!t#?u|á:8ž?}q[!t#?îÆ\ù-F?³Äèi6f?£ž0m+™?³Äèi6f?íý'±Ë?¡åðæÄaÀ?°^ǂq¥?¡åðæÄaÀ?íàiâ ÷?¢9ô }?°ü°îøGË?¢9ô }3FGL J2053.4-4052?íUÅߝ´ÜÀCä¦">jÀ:Yt^v­ÜÀ;Òù=¼¿Ä©ñÍڋI@4؃9Zë@TF__áè¿ä—I$_þ¿ß/.©9¸¿â†g1ßÃl¿ïÿÀtFEVUNASNonenone?ïŠVÖ,?–äU^Ï
¬?j9Šu?–äU^Ï
¬?Îþ?—•	\gvò?ŽÌ¾y?—•	\gvò?éøÿoðôÙ?¸ôè4¼?È@<,?¸ôè4½?îë¸[õ6¤?"[Àt{~#?¡Dz@¬•Æ?"[Àt{~"3FGL J2053.9+2922@RWâCV—À#»
QøXÀ9ÖV>Ðö'À;V±AV¥?óÙ£A«q@ŸÝq§?ø²€@LÜ¿á훨´â?ïþpßÍ@Ì?ÊGɉ1¨«¿Ùµíkí}¶UNASNonenone?뗵2î‡?¼:‡¾º¸?Á¡+‡4Eå?¼:‡¾º¸?íb']Ë\?Á8)pXéÏ?´ëí¥ê?Á8)pXéÏ?ëó8Ãm?¬‰;yîª?ÃÜ3üòK?¬‰;yîª?í"s}K;?´¥MDŸ?·kÜd¦+?´¥MDŸ3FGL J2054.3+6907@Zð¿\£@.Ÿ¾˜V£{À9ìÆ%鞕À;¤¡pþoÝ?Þ>ü³"	s@¶Š{C˜0@ªx z´Q¿ì8¦O¾ò¿—rÍËüøw¿í£­n¸š¿æ@²ôDÇUNASNonenone?çúrgêP?Èú_`
W?Ð0+Ù_?Èú_`
W?èRbe?ÐâgΆ$!?ϖ¶vkïè?ÐâgΆ$!?ë;' ©š?¬ò˜ˆp/Ï?ÀÉa}Y›?¬ò˜ˆp/Ï?؍ûaŸnº?Â3&êsÛ*?ã¹O0H¤?Â3&êsÛ*3FGL J2054.8-4908@uâ'RT`ªÀD‹«`kÀ:?ø³o.À;¹wD;Ï¿ùAž‹EîÍ@P!ˆ¬6@ސ>&¿ê%£"˜ÅM¿çLèdi_¿ÎB×Ë®iµ¿ê"gƒqäõUNASNonenone?ïÿKѲx?"úUk'?6…É°ðÓ?"úUkŒ?ïñ›¢Ù	î?f;ŽTõ?\ȺMì#¾?f;ŽTù?Þù1?‡Ìˆƒá1Å?ÈA³¸×?‡Ìˆƒá1Ã?ïÿdÍÅW?ß¡BlI?f\§Ui?ß¡Bl[3FGL J2055.6+1609@OlUÚ'(cÀ2KÈâ\
À:+òËdÀ;¢Y£àDy¿ó7‡mò÷¯@
‹fNJBº@ö_ÊëÌ¿ç
y]0¿éØyti¿â=Œ˜TJ/¿à\¢ÿã"SUNASNonenone?ïÿ5í½w?™+åBρ?BHQ<÷?™+åBϜ?ïÓó\FN?'zÌÈ#Y?vQô\ÙB?'zÌÈ#Y?ïœÿúz%Ë?ƒuÜU$¤?ˆÀavV?ƒuÜU$¤?ïýú'D?5Vƒ­³R}?7.Ç
éL?5Vƒ­³Rw3FGL J2056.3-5925@u6;%oüÀCm'Èâ]À:*¤L{ÖÀ;áà'ód?ò'ål€Ü´@óùˆl '@ir"¢?¶rj5òµ¿ãDè›pšƒ¿æ¦üP¿ïÿÒ`_'5UNASNonenone?Ïò
3
E¾?ɽâçg½?è}s<®'?ɽâçg½?½è^ëÑYº?À³"ñ¹^½?ìBô"…ÔÉ?À³"ñ¹^½?ԛŸ‰ñzc?¹=ù7¿—Ï?å²0;BÏ?¹=ù7¿—Ï?¸VCO¸˜?¢æ¢éõ:?ìõ7–ÿî?¢æ¢éõ:3FGL J2058.0+4347@U@dÜY2¿ó¬§
£3À8$óĈ[À:È	€²B?Ú¶óƒè#ã@݊µ%;@\¥ÀC|'¿ç;	XØݿ뎵jZ'Ç¿ïþh#¼?ï½IÓnãŸUNASNonenone?ì唐Àº?Áa{ruÀ>?¸ÓYëyú1?Áa{ruÀ>?æÅÍfT:?Ô!!ÛÅ?Òte2ýW‹?Ô!!ÛÅ?æ'uÒLîj?¸BRtº7?Ó±[f#+?¸BRtº7?ï%7á˜3?¦íeËÜ,?›YÌùì?¦íeËÜ,3FGL J2058.3+3729@T
™E¶ÃÀ†wc
ìRÀ90/JpfšÀ;;Ð<ÃÕ­?åðÑgñq@
ÝâÃJb@šåÀŽ¥ö¿íÀ°º¦L¿æz[>¦?+¿ÞèúÇÔ6ñ¿â]Àc÷	UNASNonenone	?ï l1ïV?Œt¥ÀQ?‡äóºÄ*b?Œt¥ÀQ?è'uVÕ?Ñ_Ž
ìW?Íö*¤«Ïð?Ñ_Ž
ìW?ìrP'é~?ªµãJêá®?¼m{p³|?ªµãJêá®?éX^_n†?²y÷¯S?ʞ‡þ'Eé?²y÷¯S3FGL J2059.9+2029@PÇQ'©"À0}°5½Q/À9öÚ˓À;…OºRvÅ¿ú&"î9.@hÛkv¹@œàŸ©¿ã²ÍN@ą¿ìr‹FÖº¿ßëtbS¿áÈAŽDUNASNonenone?ïü9ªª6?E‹À]?>7ª®Nþ?E‹À]"?ïÒÜQq?ƒ°Cڝó?vð'×vG¿?ƒ°Cڝó?D€"ß?†²Ú©ôãÁ?ŽTîßÚÈ?†²Ú©ôãÀ?ïý'½Åì??8Y4lá°e?3rОã?8Y4lá°R3FGL J2100.6-7844@s£Á½¥À@W±B,Ë:À:vë»ÛÀ;¨¥º9LR¿Õè6W!qa@éÙM
Ð@Ú]ÿ—¸¿ëF|ˆ‰m¿èⰠě¦¿ãš&É\C½¿Ý"¤[OÃUNASNonenone?ïÿ≾…>ðˆ_bòÁ–>ívAo{cß>ðˆ_bòÀü?ïìB‰ì,º?n'
ގØ?c½vÓEž?n'
ގÙ?ïÚø{ãvÊ?r( g°/Ë?rƒÂD›&?r( g°/Ë?ïöC/(?IÀ3$ÑÃÕ?SyᡯÁ&?IÀ3$ÑÃÕ3FGL J2102.8+4704@V:§›ºÜ?Òë|eVFÀ9]»JÄIqÀ:üÅCk›?é/ÇÛ÷7/@ŠaÎQ1@'ÿ\—¿åև¶¼©¿ÈšUÅô¿ãQ˜ahÙ;¿â«RyÓYUNASNonenone?î1Þ<§?®¹ÞÓ¾ò?¬ïÆ5–?®¹ÞÓ¾ò?ܢ߰W)?Ӛž‹`m?ᮐ'ÿÔl?Ӛž‹`m?ë¨_´òO?¯±Øwñôö?Á^,7¾Ç?¯±Øwñôö?è×î"bÅ?²sn¨G(?Ì Gvw ì?²sn¨G(3FGL J2104.7+2113@Q <K	êÀ0çr>á½À:\%ĵ§À;¤¬°Í"À¾|¥-Ì@Hÿœ'Ø@iÀÎO?ã߻зNG¿Õïãð!]¿èñ¾
‰"4¿­t4Cú6ÛUNASNonenone?ﮥŠÕƒ?…nbæ?"y֝JŸ=?…nbè?ïÙÃU%±£?€øaOÚ??sUm'.`?€øaOÚ@?íŠ1™¼U?£'?}Á·?³®s7'Y?£'?}Á¹?ïÿñ…w®e>ëLkôæÒ>Üõ£5À)>ëLkôæü3FGL J2107.1+2248@Q…£Â‡èÀ0V2.oÀ9ýE= óÀ;‡ÙRMI¿æå®Zk@
"÷P®ï@Ïã ¡5D¿æ–
ìZdX¿ç ^F~¶â¿è™•Rë'é¿×}‡TUNASNonenone?ïçLFÐ<3?k˜õØ
…?h³¹/ÃÍP?k˜õØ
'?ïÉ,ÙÔ÷?‡áB¬Á"Ø?{i""7Ó?‡áB¬Á"Ø?ïeDE?'yaÂԙ?žW}_?'yaÂԙ?ïìiàWV?^'V¼'?c–¨©ò?^'V¼3FGL J2108.1+5202@WTów[@ÒÜʵ›À8n†º™ÄbÀ:³×û뿼« ÜrËé@/îWŒ@v7]d¿ßëŸTR¿êöò·åV~¿ä¦ª™q*»¿îݓ»Ö}UNASNonenone?å"2+Š'?Ë$y°ðe'?Õ»›¨êÝÇ?Ë$y°ðe'?íp‡ÄÂ?ÂFADH‰?·œ{ǁÙ÷?ÂFADH‰?䥠*"Ì?·Àˆø3‹Å?×δ¿«ºh?·Àˆø3‹Å?훂´ƒÂ?«R¾
•ô±?³#ê_ãáö?«R¾
•ô±3FGL J2109.4+1437@OØ$>úèÀ5áŸâÚUÀ9NØ9¦ëÀ;"wÏDvÀ`Z"°ÔI@|p¿…¼m@ÜŸ‰Ê¿å>KïA¿ì²HČXá¿â"ÿ½ÿ™B¿æUÂ`ˆ7UNASNonenone?ïÿä@|{>î$ÿº­ë>ë¿~ƒ…F>î$ÿº­)?ïèlRB?u'!lÚŠ?g"­ð½è5?u'!lÚŒ?ïæYXM
?m'KÓÏ?iú¦§²ö*?m'KÓ½?ïÿÿ8<àö>ª\‡ç£Ù>˜øcáG­V>ª\‡ç—M3FGL J2110.0+0442@Kx"ÄGÃ
À;Ö2.oÀ:;÷ƒY¼4À;³{ë2éa¿á&æxFä@³ªÎJP[@cŸâˆ÷¿à¸94
§¿åEø(<¬¿Ù
´ë?寿ګ贒vîUNASNonenone?ïÿ©çKÅ?æG="?¹F-̄?æG=Â?ïè_Ò®?q˜ãÉ¥¼Æ?g éê-Rˆ?q˜ãÉ¥¼Å?ï³ÀÌ6ÝI?‡Ý¬t¢?ƒÌòH­­?‡Ý¬t¢?ïüN©N?7]$ülÌ/??튵NP?7]$ülÌf3FGL J2110.4+5946@X-Œ*EN@Þ͍¼ì…À9W/ ×{|À;5(ö™Nñ?ÏM٘žX+@'Ë+·é¼@EKYl-¿çõ[s"x¿ïē_e7µ?ëçÖ4÷Ñ¿ìÊÒ @3ÄUNASNonenone?îc˜¶$¿?°¬™d¢•%?©Æ´´?°¬™d¢•%?îÏ?9¨¾²?½<¸	ØLÙ?£etÚ?½<¸	ØLÙ?ë͆ lX?® ô5¨¡?ÀÉçã~N ?® ô5¨¢?&¯ï?­¯ø½¨?Ž¶T?®?­¯ø½¨3FGL J2115.2+1215@OM'#[NÛÀ8scä«æ£À:¯çÜôÀ;§Þ7X[â?×:m-n¼æ@6W'¸ÿ»@JN LO¿ã°Ì)Au¿é"Æ gƒ¿Ù¼%UÿÝJ{ñŠiUNASNonenone?ïþªË]öà?&3sf 1b?%SJ 'ýœ?&3sf 1c?ïÓDÍ"¨?"[ãZ±¼?v]ô™n¬U?"[ãZ±½?ïÉ+ÿêÔ¨?y$n‡äyy?{j
•««?y$n‡äyv?ïv†+ö'î?€ÑvaæA?'/:;\?€ÑvaæB3FGL J2116.2+4422@Uél <K
À
=›l±À9ŠáçDòÀ;J¼¼´Q?ê¶çnþTH@
œÚ–Ž¢@ô÷í¿î°±A𪿿ӺãÒ^¿ç(þ'jöï¿Ñrž<W8UNASNonenone?èI	ôtµ/?È`7‡xÔY?ÎÛØ.-+H?È`7‡xÔY?êFö'åÐD?ÎýD['Æ?Æä%¸h¾ô?ÎýD['Æ?è4aÿ	x?³kðÊ
O?Ï/¶xÚ!?³kðÊ
N?êAý|L?¼,{…ç½?ÆøŠ
ŠÓ?¼,{…ç½3FGL J2116.9+1343@P	:¼"peÀ7Ü¢G'ÝÀ:/–WZZÀ;£æÎ-¿ü½¡'	Ó@ä–'IE@ØÍ¿àVôï^OÊ¿ã²íáx-¿á}-eeé¿ê™Š]ÅUNASNonenone?ïÀ,è7xË?†j¿f	%?é‹äCšm?†j¿f	$?ïà^|¥>?y»L€¯íH?oú¡ƒZÁ¢?y»L€¯íH?ì¦ëÞoº?§¨Œ?ºÈ¡܂+?§¨Œ	?ïý9uç7_?>>"õÝ}?64PÆEd?>>"õÝ~3FGL J2118.3+5751@XcR?gôÜ@¥XÂ8õÀ9pËæÀ;d ;ë¿Ô³"î'̉@ÙM(§¾ö@Ýé_—e¿æf"suÿ¿èƒ¤ª™Ç¿ÞXœóg¿é)÷ŒáFÏUNASNonenone?ïð7&î1?h±»Œòß?_'²ü#ž¦?h±»Œòß?ï¦-a>‹R?–y4&.;?†t§°]+b?–y4&.;?îsp[:©—?Ÿ:­ªÝ*ô?¨ÈúLUfœ?Ÿ:­ªÝ*ó?ï³3åÞ?}‰Þ+Ÿ{?ƒ 3ˆz?}‰Þ+Ÿy3FGL J2120.4-1256@Cxéö©?ÀCmS?B5/À9Ô¢ç 5*À;µšTbX?äìwþÐfF@È'qßÁ@" ©ƒG¿âD4ҏµ¿ê*¯8¿æ"J®êu¿ïöEI5SUNASNonenone?ïü"‰¿)x??Ûa3?;[²´@ï??Ûa+?ïqR?"ì9£U=A?ºã»¾«X?"ì9£U=B?ïavê?"7—ËË?"Ý<¢Ÿ?"7—ËË?ëÇ;tÒ2ý?¨¾ìc+›?Àã,·4?¨¾ìc+›3FGL J2121.5-8253@sXm›äÍuÀ?M>EþÀ9ð¹£$\×À;q©Ä[åÀåèô>×@
T"ÆK(r@¤S_ùdÛ¿æ!Á½"ã'¿è…sä˓‰¿àpÓþ"ù¿éÏÐøFUNASNonenone?ïüR䐟Ã?GE;['©?=hÛ{íq?GE;['¥?ïîMnà?l.%ïID?a²'pøƒ?l.%ïID?ïȁGR?"½Ö]ÑR?ŸFï×½£?"½Ö]ÑQ?ïÿà˜Ù£m?QÑð>ïg&\"9Ä?QÑÃä3FGL J2127.1-5615@u9EÁ?ÐÐÀEÎtŸM¡À:QéõÒ"À;ÇæÿëÀH•7µ#
@
ô6¯"'®@""¿æzšûÄ\¿é¥Ù	·¿Ò³:«ˆÀ•¿ïÿÁ£›G'UNASNonenone?ïþ2D~V?D•'OB?,ßK¸™`?D•'OB?ïógý" ?e±¢Rdˆ—?Y0×ÎÀ%?e±¢Rdˆ•?ï
\Oá´}?"ÌlÖzS?ž´vÉpƒ?"ÌlÖzS?ïÿöÊÛ­5>çP-l\Ü>ÒjH¥"Ú<>çP-l\e3FGL J2127.5-6001@tê"ã¼Ó[ÀE:â–êÀ:Ç©Á/	ÙÀ<
œKû¿çš¼s°ž:@2"YŽ'©?ÿ5ºŸM¸›¿ç<íyÉ"¿Ï+@Ç+´J¿æú~˜®¯x¿Ìÿ)UNASNonenone?ïó§Œ_´r?[ð…3R"G?X°ç@—?[ð…3R"E?ïëÐ÷é{?xÍqÈ}c?d/ô…«?xÍqÈ}a?îì[?ê&?"A'CÝiÂ?¡:L]ª?"A'CÝiÃ?ïãåÅÿ£˜?gÀ&3xÃø?l:\hF?gÀ&3xÃõ3FGL J2130.4-4237@vgxÔýó¶ÀGWzÃë|»À9ŒíÀb[?À;©Äe©?ìGœÌ vå@•¼ÚçB@}´"9¼¿ãçÀ¡lh¿è"ïjÓÕÍ¿èý("Oý¼¿ïÿ¨óz÷UNASNonenone?ïÿ‹È)d?û`™à\?
<Íõ¦÷Õ?û`™àš?ïñpªÝ?g"[€Ø(?]øªEÕ(?g"[€Ø,?ïå½dÝT?ˆµÂ¯H(´?HSdUv?ˆµÂ¯H(·?ïÜá´ù|?h•æ|&•î?q%ƒAòƒ?h•æ|&•è3FGL J2131.1-6625@tjD›¥ãTÀD#")³úÀ9¦*Í3$À;Õ8¶*?òŽ1^FÝ4@©X†~߯@""_öŠ¶¿Ùî)òJhb¿ä¸pL¡ÌÌ¿éÔÑß8貿ïÿä•|¯UNASNonenone?è"','z?ÊzDÆFû?Ïçu»M¶?ÊzDÆFû?Óq*uÞi??Ëýô¡™?æGjÅË`?Ëýô¡™?Û dhžà?¹Aa_•Ñ¬?âoÍË°þ?¹Aa_•Ñ¬?Éú±_ýó?´=ÆNí?éS¨ƒ??´=ÆNí3FGL J2131.5+2605@S"wškP±À2F£"¯WÀ:)ë°½¢À;ƒŽÝ}ôø¿Û™Œ;Ê@óÝq	Øq@(¹_\±Ý?ï×*æ!va¿çÎk·mv¿åé{ÜÅ=a¿¶¿µÑ_búUNASNonenone?ï÷ïZRI?ZyÙ-6}Û?Pä!K[o'?ZyÙ-6}Ù?ïËQØñ,?ŠlOËÒk?zW‡i÷X?ŠlOËÒj?íÚº‹j?£õ¦|z˜?±*+§T¯×?£õ¦|z˜?ïð]¹$™²?[bÖ	z<J?_D¶Ìšé?[bÖ	z<H3FGL J2133.6+2821@S£ëJwÀ1Q\éåâÀ:*`	UXÀ;›•]ʶr¿ñsp/g÷‹@¤ž™ˆ§¯@üɀ'±¿ã>úµ?	¿éòµht2¿ç–]Ê¿Ðô˜PæšUNASNonenone?ïýK¤ø#?;J›™iØ0?4¢Ø>éû?;J›™iØ)?ïÓTۘ_H?ƒù¯p ?vU'3Ð\5?ƒù¯p ?ï\5:ŸR?'ó&ÊN9?ôyX¬¸?'ó&ÊN9?ïüç¬{‰?7‡€äɨ?8œ#·ß€?7‡€äÉ 3FGL J2134.5-2131@<ëÊû;u!ÀFŠœË}AtÀ9H£ÝÀ:À;¨jJ÷u¿ùñª—˜¸s@¥P+¼q`@`M¿Ø"9Ùô¿æaaÍX¿àâÍú–«ö¿Òéå,XèUNASNonenone?ï÷m5µ"'?SÌs¨P¥?Q%"•»±?SÌs¨P¦?ïóu,ˆ?dÔUµàש?Y÷¦îþE?dÔUµàצ?ïÁŒzß?"N8­¥?GÎp¤ˆ?"N8­£?ïÿ,¼÷%?!Qœ:4º?alÿ?!Qœ:4ø3FGL J2135.6+5742@XÆÂÎFI@ҒwcåÀ9Zžˆã—À;ëóف¿®×¶Ý7®6@)nu©z@ÀôÌùî¿ça
ߤb¿îM:piI›¿Á.Õu½ÇK¿ÒA»X¨…UNASNonenone?ïý#Kã­£?@_`'Y»?6å â'çç?@_`'Y«?ïIJù?Ž©¬ÊÓ4?}¦ƒ}ñ~º?Ž©¬ÊÓ4?ï¼'óå?™n~ÝîN?ÈmÁƒ_g?™n~ÝîN?ïö¥ÙÚX?OW-2ïѺ?Sð´LKNs?OW-2ïÑ­3FGL J2138.2-4939@uÀE¡ÊÀƒÀGyÔbÃC·À:,õXQÀ;^ç$?âíÊ$"w@q†žj9@W*?nªÙ¿â¼V¹ä×t¿èª9G@Ô¿æ¼þ'"¿ïùÚmZ‡œUNASNonenone?ï³àµ1·?ŒÊÒ¨Á$£?ƒÿ³'#?ŒÊÒ¨Á$£?ï1'|$º?£ÉC=¾?™Þ{{h¨?£ÉC=¿?푨³T|!?£È_	aK?³rºe\û?£È_	aK?è6f§y9?´¢Ó.‹rb?Ï&ec®?´¢Ó.‹rb3FGL J2139.5+3919@UÐ?'æFñÀ#бx³pÀ9›ó÷´$À;}ý¬h©?ð¥\ürÖ@+ƶ³/î@ƒ¦¹Ù«¿ëÑâÔ1V¿å'Á³`Œ¿àª­<±¹¿ã>›¥ÂUNASNonenone	?ï}ïþÑݽ?•'µø·?B%ÄHT?•'µø·?ç§Ø3š?ÑÍéÇ_ý?аO˜ÞÄÍ?ÑÍéÇ_ý?êÆ×¾{L?®M0¡vµ?Ä䣩Ó?®M0¡v¶?ä}Bÿ›Û?»A–…?×{îÈL?»A–…3FGL J2142.6-2029@?$i@5z5ÀGG@Ý?á—À:å¡Ý4ùÝÀ;Ά"W£?ä¤õ߯lY@
Ö3=o!K?ø[6CÌÞ¿ÜàÃ2f§¿à"ð&½ü¿ïÿƒb½?ïÿH
úƒXUNASNonenone?ïÎqô0Ã?…À.]*hž?xÇz瞚?…À.]*h?ïîE9W'Ù?v6'`ÔU?aºÆ¨n'm?v6'`ÔV?ëgz²yõÜ?­¶Ã2OaX?Âb6(?­¶Ã2OaX?ïqÈ+ƒâð? J›¦4Át?'Æúƒ¢"? J›¦4Át3FGL J2142.7+1957@Rnì€Ç:½À8dv}4ßÀ:±<¼M#À;ÝGP ©Ä¿âjaj©9@
Ü7ùÁx@ÆÿXeG¿î(ÂX¿Þÿhd‡,ô?Æ;4}¸	¿çxšö]UNASNonenone?ïúâ$¶j?QVd©°Ï?DwmÉ&Y¬?QVd©°Î?ïßx΍µ§?z"ÐÇü½?pC˜¹%,Ð?z"ÐÇü½?ï~µí}·?ŠØ,"x?ô?)\âPI?ŠØ,"x?õ?ïøÿ"4?VxEö—L?L­¿ç.¦?VxEö—L3FGL J2144.6-5640@u8}¿HÀFßÓÃa@À:œF&Tþ_À;¹ÌÏQ‹?êÔ¥ý¼?@až½c£@¨j¥§š¿ë'FcM¿ìdG"EL?¸YØxýlÓ¿Æ\Z®î"UNASNonenone?ïþ«RáH×?2½5ƒn?%JÑër'?2½5ƒ\?ïñêÿì?gûxN%Cw?]ËÎ*+V?gûxN%Cy?î'BÄäÁ	?šªë{P?¦ÛÓ±³ïl?šªë{O?ï¤oÔÓ§?ŒZé‹q?†ä
ÿ?ŒZé‹q3FGL J2144.6+6606@Za¼@ŽÉ@#ˆdüÀ9Óz¬nˆtÀ;ŠÎû{6ÀQ*3d>@7å´™@¤ÿŸÝÖ_¿èz^ò\¿æ¥6û꜖¿ê‰Q"Eä*¿³Ô~.õ…UNASNonenone?ïè eã'?k¿óÜ{ë?g_åšÙÔ?k¿óÜ{ë?ïà7à Éù?€T5ª+?oÈ_6N?€T5ª*?œpø\?™üÈM"šÈ?¥–8ðzC?™üÈM"šÇ?ïÿêÛ^%9>ñOãKÕ>>å$¡ÚÆ¢²>ñOãKÕ23FGL J2145.5+1007@Pƒ:'£À?‰Å«âqÀ:žÉã%ÕÀ;ºF"
q?ØøšJŸ@
%Â4‰´?ø××?A‰b¿ïĸ#G'Ë?èF"y&²q?´pUñÍ¿ºî‰FKz
UNASNonenone?ïþäQ_\z?%9Œ»/?!ºê
8l
?%9Œ»/u?ïé3œ?q^Î¥AÈ¥?fÌ=pëdª?q^Î¥AÈ£?ï‡É­]Ž‰?…ÏwƱL?Ž
"¨œ]Ë?…ÏwƱL?ïßXJ¦8?lÙo´œ"?pSÚ¬ãôî?lÙo´œ"3FGL J2147.2+4730c@Wnõs}¦Àk¢æIvÀ9"La…VÀ;6É5h—™?ãÓä(^@
Vu´¶@w‹¿ç60¿â(ÙcÅ2‹¿åûhk¤=â¿è¢'ð'ßn¿ïþŠ¿·¡UNASNonenone8?æ쬥§¶?ÉJñ]ëð?Ò&¦µô°"?ÉJñ]ëð?Ñ0g´õ¶?Ða"ýyž@?çtçÌ%…%?Ða"ýyž@?çËäãú?´,"|ൄ?Ðh69óô?´,"|൅?ÙЯ®2I?¸ èEàíž?ã¨(æü\?¸ èEàíž3FGL J2150.5-1754@AѺ^5?}ÀGºCªy»®À9¯[¿PãÀ;¸@p"Í¿¿J‡C3d@\>ø8`o@Evå¿èFì‡'Q¿ìÜìÌéË¿ÜMÓ4<j¿é	¿ônž¼UNASNonenone?ïÿM;È?OBñb4?X†þ>"á?OBñb4?ïíjâã]³?klÂ6ƒ?b•¢M?klÂ6ƒ?ï¹ÞøXß®? ŽøŽÈÆ?ˆAéȨ? ŽøŽÈÃ?ïÅî­`m?p‹V`ÀÇ$?}ö©OÉÉ?p‹V`ÀÇ%3FGL J2151.6+4154@V­ó¶E¡ËÀ"åÈ23XóÀ9°ÏS(œÀ;jV9Èxª?ç;™|Ïo¦@(ZÅ4¨?ý"ˆ`Xy?ïÅÛýþYH?Á7†""0ý¿áö7™¿Ñ—ÔtAUNASNonenone?ïJ›&µü?Ÿ×3ýͯà?ž¬›)@x?Ÿ×3ýͯá?êkÅǼ²?Ï"τ™ìL?ÆSðèá
5?Ï"τ™ìL?íÜçsBVÒ? mLRŸ?±ÄeíIp? mLRž?ç~‹¹×?¿ÔrrÛ°?ÑÁèŒQÝ?¿ÔrrÛ°3FGL J2153.9+6626@Zž†ƒ<`@"ÚÚUK‹ðÀ9²Š½]ÄÀ;%ôß:›¿Ù]W…3A\@–"t¼@5_®ç4?źÚ
fпàWågÎE¿îÀ°^×ý?¯#³=£‡UNASNonenone?îÛ9Á"eM?ªÛp8X6ÿ?¢LcæÉ«-?ªÛp8X6þ?︂îØ_²?›@D~½?ßDIèE?›@D~½?ë8>R­6Ì?¯
Æ·m_?õK$Ï?¯
Æ·m_?ïЕÛ0Øg?y"â+£c?wµg"Ì?y"â+£d3FGL J2200.0-6930@tö"Fs'ÀD{ꁺÀ9°Úx†ú[À;À‡»JÄI¿Ýjá€Õ@
µ"}¥ó@Î
Ÿ–2Ý¿éŽýCô¿à7ðeiwy¿éÛ(I+¿ì9Š¹	ªUNASNonenone?éâ{dºð?Á*Ýpl¿ö?Èwòm=?Á*Ýpl¿ö?îöû?Qîá?°šUŒ·? L
áå?°šUŒ·?ëþ½I?¬üªèð²L?ÃÇÀÁ
Û?¬üªèð²K?î{ýf¡?Ÿé'Í%?¨@)•îæ0?Ÿé'Í%3FGL J2205.9-4704@uàÛv³¼ÀJ•=êFZÀ:RhDŒ÷ËÀ;ç&p­F?㋖͝"_@
¡rŒÖ@OÀ A¿ì@%"0›v¿çÿ–VKÄ­¿Ô›ã<óå¿ê??\¦
	UNASNonenone?ïó"©Y´?a=¹±ÛÞÓ?X×À­L•Ë?a=¹±ÛÞÒ?ï¤ä¼e;S?ó<?Ðs?†ÆÐæ±+-?ó<?Ðs?îÂëÆ.üž?—cÂEýZ>?£ÑC6?—cÂEýZ>?ì7Εö×d?±=è±·Ç-?¾A‹PIDß?±=è±·Ç-3FGL J2209.0+3652@V5*"8	À.ûBªŸ{[À9Ýã‹U38À;ª€÷â$M?Ä*½ðs@
¦zÐ֜¯@±Ø@žUÁ¿éùö˛@Û¿íÈnµ%¢¿É$ŒÅSd_¿ß&Yÿ»UNASNonenone?ïùhᴞÁ?PÐÛÛo¿I?J\y-"þê?PÐÛÛo¿K?ï€$,MàB?¥ÛúÊ;%Ó?öôì‡ï‹?¥ÛúÊ;%Ô?ïxY½¢1°?‹YH3Þ§?ôÈK¹Éà?‹YH3Þ§?ï˜c¼"ð?Wú9Å`?‰ÿ'÷D?Wú9Å_3FGL J2209.8-0450@K׺Âß
AÀFÇvõ׈À:--U£ "À;eÁsÓ6s?çÒR:èç¾@]ûÞ³)?ôA»¿3\#¿"¨ÚúîæV¿ã¾6ÿæX(këÔ?¶÷›CÈÆUNASNonenone?ï«!…?ŠmêÁ±°ô?…=÷º¿/?ŠmêÁ±°ô?ï펌9¦h?s03YžR¸?bqsÆY—Ù?s03YžR·?ëkšQƒ?¯jÁ"Åì?ÂS©—Ò¹ó?¯jÁ"Åì?ïQK‹iç?"q-¤F¢ü?•Ý6Ž'Ã?"q-¤F¢ü3FGL J2210.1+5925@YëäO QD@Àc'†WÀ8œzšÐÑ>À:æRxrØe?ìÌ;5œUG@0–Jښ@üVàŒr?¿á¸VCT¿éF'ì‹¿í¤ˆ3{闿îIšt¤±jUNASNonenone?æKìºb7æ?Ì!uMΌ?Óh&‹;4?Ì!uM΋?ÁÂÕoÂ|ç?Éöç"-ó?ëJ¤`Æ?Éöç"-ó?á0žjPÈ?ºžö§«9?ݞÃ+ï^q?ºžö§«9?Ãn×
¤V?«êÂõ¹Ó?ë$J=Vûj?«êÂõ¹Ô3FGL J2210.1+6043@Z=îx@@AéÿãzŽÀ9Ë…ãpÀ:Ö8Ûé B?ÕÛNt®@gAžÛÍÇ@´ò€e–¿çý%ôËj¿ïÿíb»ÙW?ïüÎδü¿Ñ$|bßUNASNonenone?ïÌ'N?",>*:Æ?yðÿ·Xõu?",>*:Æ?︫W"m?'{ív-[_?Õ*<[$¹?'{ív-[_?íx40˜"?«ôëV糃?´>^{?†ò?«ôëV糂?ïñ9K|Éw?ôŎùÉ?]imÑ?ôŎùÊ3FGL J2210.2+6509@ZÁøL­W¼@–*"Š>À9ƒžòžîmÀ:̍Wk÷ ?Ú¿Ýs–®5@áQ•sð@ϧŬ¿è'+f¾®…¿ëŽ´Ô©˜¿ç""
Ó2¿ÂÆ!{¿'ÑUNASNonenone?íªýí}3?º½g$µí?²¨—|f?º½g$µí?ïb;îÃY?«éï"P?"¸Ÿâ'"Ú?«éï"P?êµЯF?¸çôBÞD?ÇÅ+"½Bç?¸çôBÞCÿ?î›áñš2/?¡íœDõÿ?¦Aàæ\Ý?¡íœDõþ3FGL J2215.5+6122@ZV~ùÛ"Ñ@™l?Ä;.À9Ó'YáÀ:Ég¦†é?òíȀþç@
Q[ÅM§~@;¿Ý/ñ¿Ò±kã(þ¿çèFiµ•¿ë…ü~ ¨¿å'ph]¯UNASNonenone?¾ϜŒ‹?ÃaOz.±?ì?_no?ÃaOz.±?ã¶~¬!Àq?Ö©õèÓ?ؓ§¼ ?Ö©õèÓ?ÙóÃæ2 ´?½Œà‹#é
?ã毦?½Œà‹#é
?ÂJä#ØM?±	Ç_øÈ?ëm|Æ÷	î?±	Ç_øÇ3FGL J2217.2+6346@Z·#c²W@KpïVd'À92ÀÁ%ϝÀ:ïµk‡7—?ÙÒ
	ª^õ@
>>lLYu@v/ŸTïq¿ÁøÄË)<B¿èîaœýý¿å¨øál…Ô¿ãS'æ&]UNASNonenone?藔Ò݇?Ê<*Æø¼?Í¡¬´‰áú?Ê<*Æø¼?í÷Xãûñ:?¾ aC‹
ñ?°E8à v-?¾ aC‹
ñ?脌•Í°(?»ä»·¿Wú?ÍíͨÉ?_?»ä»·¿Wù?êJ{Çu¶3?²~'ûØ?ÆÖâ)'0?²~'ûØ3FGL J2217.8+3207@V3RÒ4ëšÀ4_¢œwškÀ:Jß72œ4À;Æ|°TÇ¿ê©ù>a˜@¬Äĕ›³@(_o§-¿åØû)xí¿åÛr…¿®<¿æcY·_ü¿â*Ûì'þ*UNASNonenone?ïßå³(1?w
ZåqC?p
&kçyê?w
ZåqD?ïªuÁÌÖý?"w|ØŒ?…bŒÊ@¬?"w|؍?îâ´
#žw?•&èÔòT?¡Ô¿-Æž?•&èÔòS?ïÏÀñJ¡;?r«4¹X('?x‡Z¯b?r«4¹X("3FGL J2220.6-6833@t»ƒÏ,ùÀE~s>»ýrÀ:p'Á—åÀ;úIŽ¿K?Á3ÎCoks@UQŽ&ô@
`V,?¼ôty­¹¿¿#H¼SÐ.¿ä­>!MØ{¿âiØd
NPUNASNonenone?ïàYùó-˜?SL \Z)?o¦ÒgÓ?SL \Z+?ïçýò]Ó?q¥ð1…«¼?h
¢ë-?q¥ð1…«»?î¨^·M¤?œu!È»O4?¥z‹%¿?œu!È»O4?ïŠþŽl›å?Zrù¾_&?@\dÙ¸?Zrù¾_%3FGL J2223.3+0103@PMÔA5TvÀFL\|ؙÀ:>}—ÛSxÀ;­?)
»E?ÌÀ™~§â@
Ñìšó`à?üðxá=G3?ŗÊeÙ˜¿á½'œ¹Î¿¯"ç<Ü÷Š¿Þçg¾çB*UNASNonenone?ï÷"±N"C?Rëã&t?P֝c»z?Rëã&t
?ïï%§õT?i$W}æ?`ÚæX
«?i$W}ã?ïw š#Ä
?ˆªšnCf*?'컇~±?ˆªšnCf'?ïȐ^Rn?rÍ52)—?{·ÐÖÈÿú?rÍ52)—3FGL J2224.4+0351@QšmÚÏÀEsG0@9¬À:sˆ¾€À;§¤&»U¬¿É'6G~ˆ‹@HtÓ¼€#?ù‡µ'm,?ïü6Ìq'¿àà~~ú˧¿áÿx÷žÄ?Ĩ0A\ŽUNASNonenone?ïþå!¿wŽ?$´ƒ•K?!­ä‡R?$´ƒ•K­?ïò7•^2?ez#¨PO?[ÕC›âV?ez#¨PM?ïb¨´ù6?‹W÷;ºÆ?"ªé|Ù:?‹W÷;ºÈ?ïô÷;=˜ ?TZ°iáØ?V‰"ο¶?TZ°iáÓ3FGL J2228.5-1636@Ew}XÀK®ðà¨KäÀ:&êÓ²šÀ;¾Îf*…?ã'ó¬Nkã@<k›"€X@
Y ,Æ2¿ê£Oÿ'蹿äDn[¿å^gæ‡ø¡¿Ú·ï-}oJUNASNonenone?ïú@è½!?Iá!*š­m?Fÿè]Í?Iá!*š­p?ïíή(‰?lÿi:ͬ?b1Q×þv·?lÿi:Í­?î¹>9e'Z?›àåkõ?¤li§Ú\?›àåkõ?ˆ^?—JL•Þu?¤g—Žª(?—JL•Þu3FGL J2229.1+2255@UB>ÕÀ=FژgjrÀ:9^>y¸SÀ;ÊPg÷`¿ÎnÝ	@Oðò'@é®@o±¿¿åüCà‡¿ãù!3¶¿és¤¦©M¿®µÎCõl6UNASNonenone?ïÝÿj곖?wúGJk"(?qJŠ¦59?wúGJk"*?ïäÖàNÏÙ?t˜®Õã?k)±0&É?t˜®Õä?î›íUH.u?œÝ•å[³H?¦A*«}ª?œÝ•å[³I?ï؜Ç|R?pOÍöT«?s±œA¹Vü?pOÍöT«3FGL J2237.5-8326@s3"µÜÆ?À@DÈ`VíÀ9¥"L["fÀ;6dÃÎ÷?àŸñgêR¢@¾æåÒ­7@x4€3>¿çð¥ë>.¿â5v{Ô¯¿æûFf…‰Ü¿îVP.@°UNASNonenone?èqÜdL,–?Ō$5Ju?Î8ŽnÏM«?Ō$5Ju?ï4tnDÁ5?¦K44x•Å?™qr7gÙJ?¦K44x•Å?æþåÀ‰¡†?¹_¼Va?Ò4~ì¼ô?¹_¼Va?ên†Ó#´ª?¯o)Þó¶y?ÆEä³q-X?¯o)Þó¶y3FGL J2244.6+2503@Vpڐî¢À=ˆb¡µÇÎÀ:§x+ŠÈÀ;æ<³åu?éÉÇè?!²@
Õíðˆéž?þ¶1_žv"?Ü*Ž'?µO˜©
¤¿ÕQ:í^45¿à¢Ou´7UNASNonenone?ïÖñ6D•—?|˜_/!m?t‡dݵ4ž?|˜_/!m?ï±LíŽ?ã.mo3?ƒ¬ÄœW?ã.mo2?îârlÀT?•òÍ°ð+Æ?¡ØÙ3ú¿á?•òÍ°ð+Å?í§èLD?¡d,(€ƒ?´ÇȽÙ?¡d,(€ƒ3FGL J2247.2-0004@QÂÀð ÀHÞbäѦÀ9åóìÌÀ;›z6'?Ëøòd•x@	E—丧@Ü·àð?¿b v°¿æûÒp¥¿àÞ+ÿ7X¿à,_ÃEJÉUNASNonenone?ïýMT=ä?7…JdU?7]•^ی?7…Jdb?ïë´Cì°?nyè"ñà?døK¼O;?nyè"ñß?ï~	)€"?Š¯ƒ¿_)[??ÚÏí…?Š¯ƒ¿_)\?ïb3¸óÇ?°ò;áiÞ?"¹ˆð‡+?°ò;áiÝ3FGL J2249.3-5943@tqŒ½D¦ÀI¥¶…ì>À:åwo£&
À<'Y
]QÀè>WÔ}E@
ŠÓÒO˜š@dhÀí_¿æ;Ïl—á¿ÖËÑǀ¿êêu'°"S?ÈKÕI%ÁcUNASNonenone?ï¯z'SB?•úvÝÙÊ0?"!_k<ïƒ?•úvÝÙÊ0?ïôyÁêž?c¥Ý
^7?W|+âÅé?c¥Ý
^7?íi{
ۛ³?©ˆˆµ=ð¯?´´'©#"d?©ˆˆµ=ð¯?ïÿõ©²V—>ÝÇ(jç&ã>Ô¬›RÑx™>ÝÇ(jç*°3FGL J2250.3+1747@U–ª:э&ÀB*R¤ À95Õ"äFÀ:ë°Š`A¿×¡³†!9-@ݽ=¸@@H)`vP¿ê¹ý¯:7+¿æ~@–âÉÓ¿îìbïŽmÁ?á8¶ªCUNASNonenone?ïÿY»º¯?!X¦j£šg?ވˆª$ö?!X¦j£š$?ïñ'´d'?gK¬­¼?]Í°—7²P?gK¬­¼?òÕ.÷?¢rªJŠ'p?¦tðÒ­™?¢rªJŠ'p?ïÿy¹×£?K
ª·§?ÈÅ
ë¤y?K
ª·§-3FGL J2250.6+3308@WêÝëÙÀ7AÐúX÷À9ø8¢Þ¼¹À;Åß3מ?ó3¥^sÓ·@
êr$4¾@ÕãÿÄEë?ÜdR5¾)¿æ>k‹nó¿éΏ¿Q¿ïÿÙUNASNonenone?áSCŒ[?ÑMèKR?ÝÙýYxçJ?ÑMèKR?±ø:‡Á·s?¸h¨X°5?íÀø¯É?¸h¨X°5?Û1Hº.bú?·¼Y'¨?âg[¢è΄?·¼Y'¨?µn…–)? HU†ÕÆ×?íR/M?ŒZ? HU†ÕÆ×3FGL J2253.1-1237@K\bõ˜ñÀMb"aùðÀ:$tÎÀ;ÖËÒÑɌ?îy‡ôom@¥Ô/^@‰åÿά̿ØeöÕ¿èud¤«µ¿ç1ÉÓ7
ø¿ïÁRÿx¾UNASNonenone?ëi>Lë?Àߘ^ƒÈB?Â[ÌS·ð?Àߘ^ƒÈB?éÊ2?]0¦?Åò:ÑSº?È×7‹=h?Åò:ÑSº?é2.s,kß?³õ­VÄú#?Ë7F3NP‡?³õ­VÄú"?×~j­)X?·£u@#?ä@¿J©kT?·£u@#3FGL J2254.1+6229@[v"8…
@ ݂ýuâÀ8ÈI°M:EÀ;Gckà#?ÜÉhÚ	 e@A⹞ß@}_Ò"¢¿áßZËuU¿éö¾á¿é#Y…ú¢À¿ç§2ŋKUNASNonenone?ïÓt "C?"â˜lâ?‹"÷ÞïI?"â˜lã?éŸ'o
?ÎH.ru†?˓™¶C×?ÎH.ru†?ꥌÛSsj?´°öþÉ?Åi̒²2V?´°öþÉ?èØo)\Ь?³É·Ò?̞CZŒ½M?³É·Ò3FGL J2254.6+4253@YM†DR?hÀ."'›ØÀ9µr҅srÀ;"=?%¯½?àFqï0¤ã@ލz&@FHö…X¿æ]ÓèŸç¿ç`XUŠ(Á¿éèx'{M‡¿ïÿ–ȦCîUNASNonenone?ï'7‰kØ/?'µ¿µ€?‹r¥	ô;?'µ¿µ€?å\©˜NVß?ÐTԂ½îŒ?ÕF¬ÏcR??ÐTԂ½î‹?íò‰†¯v"?¢ñ†B?°k³Ê"Kã?¢ñ†B?ãE€Ö¢Õ?·q­dz"?ÙtþR»ÀT?·q­dz"3FGL J2258.2-3645@8R÷ô˜ÄÀP$³=¯ŽÀ:¿Â"À;ïìì'(¿²œN˜lÝ@29Ÿˆñ×?ÿKA¿½ð'¿ãá•5¶C?Àe[é«f¿îÃnšµ?è«é‡ˆÊUNASNonenone?ï×G(³'ï?ϊ©lh?t\k¦l–?ϊ©lj?ïóTºëñ?e"™›g
«?YV‹ø(‰?e"™›g
¬?î»0j-/?¡$"–5U?¯Lù]-?¡$"–5U?ïáÿ,oÔ-?vŒ>Hðt?nӐ+Ò®?vŒ>Hðt3FGL J2258.8+2437@W.~ùÛ"ÑÀ?­W¼xÀ:ÈB#'À;š‰;}"¿ñœÝø©Ê@¥n‰ }9@xO #¶é¿ä¶_ ˆÿ¿îŽ:üçX?ÌÕp'î¿çQù¶©UNASNonenone?ïÿâÒoù>íGäcw\>ío-Bb>íGäcvû?ïí첬)g?lJ+³éO?bMS֘Ç?lJ+³éK?ïҍ!rÓ?tԏqϹ?v¹oFñ–N?tԏqϹ?ïÿ•î¡rb?'.}Ÿç?
"W£gyj?'.}Ÿ±3FGL J2259.9-1553@IXÜìÀNëD$>ûÀ:O&ËEäÀ;ãpûÞ´?çrÝæƒ4Ü@&î'm¦!@å®À>•¿ÞÏ
Ž¿à>íÚ?¿â"%¸«¿è*‡= UNASNonenone?ïÁ­³šQß?4á>7)?)&2×7?4á>7)?ãk2?'›ª'Ó]?ˆºG%3œ?'›ª'Ó]?í÷]¬
3?¢­ë2ˆ?°EŸ—†i?¢­ë2ˆ?ê/,OYdD?­»E§ƒi?ÇCNšnò?­»E§ƒi3FGL J2300.0+4053@YO‰ 'RTÀ1>%Øם
À:5D…kÀ;®ÖuÂú¼ÀøBÃIs@¹®@ð‹?ø9	Ü¿ïØfNq/Ì?îßë5v7¿ìÕ&sÃW?éV¸MäºTUNASNonenone?ïÜáÇې‹?yÃ?r¬†K?q7º?yÃ?r¬†L?ïۂW½¦?€Nm‡áÅ?r>Ô!},Ã?€Nm‡áÅ?îçJ€§J? -¢"Ï"þ?®1‹Wõ‹W? -¢"Ï"þ?ïÿüì,$j>ґ"i·®[>¸žžÜ«Ù>ґ"i·²3FGL J2300.1-3547@…Ø=CWnÀP66ŸÏ=ÀÀ:Iæ¯ÌâÀ;ðXr‡ÜÙ¿æ
zßwÓ@FEêE¾@z7?‡Ts?çh\eþÚ¿æpÙquä¿ãlŠ2¿â…f®'+`UNASNonenone?ïÿˆ€"wŽ?Ý/'6ø;?
ßÚâei?Ý/'6ø`?ïó³ºÉr;?cò»[¯lr?X˜Šmˆ+?cò»[¯lr?ò¶¡ø?"çFÊ&éc?ŠCRWù?"çFÊ&éb?ïùO€[þ?E…
9—?K¾Áþà?E…
9—3FGL J2303.7+5555@[
…Æ}þÀÃ@&`¼ÙÀ:@»â™½¬À;œÜD9õ?è»[.ò(@
Z[k5®?ü‰Ÿ¦xû¿Ü1튩ß?ïû­9ÙH¿×þ}êªr¿ä
4Ô?>UNASNonenone?ï¨ûydü?Šc-!NÛ?…Á!¼&Á/?Šc-!NÛ?㨻^NÙ?Óc{"¸^m?د‰CbN?Óc{"¸^m?î©Â¢ÂÖK?™ÒV6‹e?¥cÕÓқO?™ÒV6‹d?ç"[¯ht?»ª	âq?Ð÷IÄ¡/?»ª	âq3FGL J2305.8+1658@Vqn?x»ÔÀC€¡UO¾À9Ø+{¯À;Aù¬ÿ§ë?҇‹-ŸÝ@´l8~L@3Œ¼¿éÌý°U®ï¿ì5 æO¿Úæ`æ¹vȿ纕KÅêõUNASNonenone?ïÿ×´›]>ôLÃÉC¹>ô%²Quy«>ôLÃÉDå?ïîS¬–w?j#l­¹¶?a¬Sài‰p?j#l­¹¶ ?ïÔa—~rž?x«Cq•×?uÏ4@Ʊ
?x«Cq•Ô?ïÅ8
ÞäH?q¯æ€ßµÞ?}cúÜ/?q¯æ€ßµÞ3FGL J2309.0+5428@[}VlôÀÚüGä› À:Ž¯à,üÀ;¯§Í9WÀ:$¾ü*@<9·[ÌZ?û('¿/«>?ïÿ/FOÖ¾¿áî$gà±S¿ê+ÛjjN?Î_É4
UNASNonenone?ïåâ
Ö¢…?o$#4÷—F?jõ)]{?o$#4÷—I?ïtTwø4B?¤n!uÑûB?'uqùw«?¤n!uÑûB?í[ïD×?¤Â%@N?µ ‡íßùF?¤Â%@N?ïÿë‰Ï$é>ôMà&¬"S>äv0Û¬>ôMà&¬ƒ³3FGL J2313.1+3935@YÃxFÜ]À3uº² À9úò03¤rÀ;º7'´yð¿îñØ@I·yS~@Xk 7™¿éD©Qü¿êÀ›ñ¸"‡¿æPü¸*†ð¿Ô¢[oéUNASNonenone?ïüƒp¯)?C@¤l¾³)?;ãôz†²¾?C@¤l¾³.?ïÑ11Ø%Â?'Ê?x|Ãp?wggí‹?'Ê?x|Ãp?ïŒâ»®Ô?†síH?ŒüQK?†síH
?ïý °ç™O?0Áo _Þ?2úxÃ5ˆÝ?0Áo _ÿ3FGL J2318.6-3829@vKÂã>ÿÀPáú~¶¿DÀ:Cê¡ô²À;úWâ?$Ù¿â"D‡»Ã@
Ò9u—‡@¡ß¹8›¿ã_'»Ëj¿áÑ)¨<l¿ásŠƒH–¿¿ïÿúw2šUNASNonenone?ïëB)ÚÓ?u®Ë²8¿_?dþ½Ö%.?u®Ë²8¿_?ï´]ºš."?'qnU•?'è'Ytw‹?'qnU•?ì½I'ò?ª3Ofê)G?º/-³èm?ª3Ofê)F?ï"è'D$?ƒãæäc!G?‹ø[n÷
?ƒãæäc!H3FGL J2321.3+5113@[7ÙÓEŒÒÀ"Yò™0À:ƒ¯'R£;À;Åú¬(©¿òSdvL7'@
XÕȞê¼@&ˆ "ä¿âm
&õbB¿ç¡˜Á'l¿ÇÏÿc-f¿áÅÐÚ#UNASNonenone?ïü*>mã?C©@ÌÅû?>«ê©?C©@ÌÆ?ïxÇjH°Z?¡rñ›ØØê?ç¶éô¡?¡rñ›ØØé?ï½~BÇÖy?S<"ÜÀ›?€ oN
a×?S<"ÜÀ˜?ïþ/²ß›0?0…Öб?-ÒLý%?0…ÖШ3FGL J2321.6-1619@KßÕÃÀP¤yèQÀ:Óe
 ÒsÀ;ÕSV¿)v¿;oX» …@
H€´ãw?ø†D 
é¿ïÿG+À^?ïÜèêi?à_ÝKRÂM¿âI:0¨iUNASNonenone?ïÿÚö"?"ýlÖѕ?"½!-sœ?"ýlÖх?ïðÌã‰Ô‹?q®fèðö?^f8ìVëy?q®fèðô?ïp¸§zZ;?rI.3¿?'èë´¸¡?rI.3Á?ïõŠTwl¦?zËq¨oâ?TëW&²à?zËq¨oã3FGL J2323.7+2523@XÇP%"õÀ@²õýG¾ÛÀ:{—)|ÑÀ;â%™È"¿å=äiÌwg@gGPvÿ@__¶ôÉ¿è?+~UgÞ¿Ü«'GËú¿Þ"ZT®ä¿â1@1ôDUNASNonenone?ïÿ9@º§Å?'Úˆí— ?×è«_,?'Úˆí—-?ïìM…|·?må³)°?w?c²ízƒH«?må³)°?w?ïÉrh9Ks?yŠn XfÞ?{FËãZFð?yŠn Xfà?ïú
Ó?AïÖ2XV'?GËû‡Ð´ä?AïÖ2XV£3FGL J2327.2-4130@uºü"µÜÆÀP㦠YŸÀ:LÚ")=À;¬sWæpã?Áa^68˜š@µîŒ:5†@4Ý ·0¿ä¬ÍlÍ¿äºà恡"¿ë1pΧËê¿àØ-ÚóoéUNASNonenone?ïų›}Ȕ?ƒ­UyÄf?}&2Aµ¹?ƒ­UyÄf?﫬«1¯š?™§în¯@Ò?…Õ3"²?™§în¯@Ò?î	ú.%?ŸæîŸJ?¯`W
]½?ŸæîŸJ?ëÌ\"Bú?°©ræµÃ?À΍³ºô?°©ræµÃ3FGL J2329.8+6102@\M¶°_¯¿Òê~8•À9®ç¸5À;D
ð
­¿ç²9´¾@
:EÌ@|y ç¿è`ÎۚƿålMPjх¿ÇR!ïدH¿â¯3ŒUNASNonenone?ïü`
˜–?>ÞÐæ¤R
?<ÿ";OSç?>ÞÐæ¤R-?éi}³P?ÒuÎsç€?É¿ÆZ	2Ã?ÒuÎsç€?ïõjO?Šåïù ™N?R¶\K?Šåïù ™K?ïö5kē?U·¢ièº?S•)Övه?U·¢iè³3FGL J2331.9-1609@MÒR'ƒÓ_ÀQ$GÃ
0jÀ:5õáõSÀ;ç"6Æf?íEförý<@%Ƃýk@SÐ@Ô?éãÁ^¥…¿àK¯"dP¿Þ¥Y¨ŠD´¿ïôÃaû-ïUNASNonenone?î"ëw?³OZ"Éüp?¯±OH˜?³OZ"Éüp?ìÉD¿ŸË
?Á`ïÖâc`?¹µÚ§­?Á`ïÖâc_?欈Tš5?´äÂ#~F?Ò¦ïVËõ–?´äÂ#~F?ç+l«¤ÖX?ºƒüµǀ?Ñ©&¨¶SP?ºƒüµǀ3FGL J2333.0-5525@tC"Ðå`BÀM,k΅3±À9Ñï<c]À;ë›
ß½?í·&ÑaBK@
ð»äó	M@Åh`'6¿ÝèTZÓ¾·¿âïM,¿áéBËùày¿ïÿá_¥UNASNonenone?ↂ¾î+?ÐN³hº'?Úòúz'#©?ÐN³hº'?Ôöµ­U
?Ò]9!S•æ?å"û¥)U{?Ò]9!S•æ?âeWW/8?¹üÂåûq?Û5QQ¡ÿ?¹üÂåûq?Ð81t?¶bºF4?çùãç~Eõ?¶bºF43FGL J2334.4-7948@s1³g ù	ÀBX—{žÀ:OŽR=ºvÀ;ÃÍ¡Þâ?Çâ|_T¬Þ@ºý¡Uü@ø¨™Mn¿è›Ñ¯à'â¿ìitònƒ¿Ð½TÁMh¿æ
åH UUNASNonenone?ïÿ"ÆTÎ?šÖ
šã?Îj̕Å?šÖ
šŸ?ï½à!°?š½wßXJ!?€‡ø÷"ßú?š½wßXJ!?'-¶?†øýˆ?Ž\Û¿t'x?†øýˆ?îÞœq;?–†J¸w£?¢–8ìL?–†J¸w¤3FGL J2335.6-2342@DW´ÀR#¶þ.n¨À:PJ›.ÅÀ;Ø*>—ëD¿ñ#†TÃPÍ@×8Ëùh6@-à_PÈ¿åÍ¹¿èy1ÈÇ¿éwíÒ"nŒ¿ß#<*R¹áUNASNonenone?ïæC?—"?rDÝñR§¾?i¼ÀïhÝÿ?rDÝñR§½?ïíÿ'*5?s˜xªý+?búØÕÊ?s˜xªý+?vk;}?šAˆàt9{?§¸™LH2?šAˆàt9|?ïÜ@ÍåÚ9?oþ¹-Ð?qߙ
ãœ?oþ¹-Ð3FGL J2337.2-8425@s}ŠüÀ@3EbàŸèÀ:v"Z»7À;¬1u¿¾ÚS"´,@
C˜LgŒ¬@ ­`uᄿÔΣUt¿æ;º{ïî¿èì|•å…?ÏwžëUNASNonenone?ïÜ!r=RÏ?vöÌl_UÁ?qïFáV˜¦?vöÌl_UÁ?ïß[íó¶?…×۟F,?pR	w$È?…×۟F,?í
‰`PR?©1pã7§M?·"´ý}o?©1pã7§M?ï'j¼áÙå?Š£ñ±ƒ?‹ePlj†ž?Š£ñ±ƒ3FGL J2337.5+4108@[ÓØYÈÉÀ3ž¢	ª£­À:eÉÞÜÀ;Д9ˆŠ?Å+á×¢@@&Ít<"@ÎçßwÊ<¿Ý!.üö=è¿ìÈöÑ$—±?ÙJ»	ÖÃq¿í–©C'ŒUNASNonenone?ïU+ð'?§¢'â±uô?5ZíÌw?§¢'â±uô?î'—¿r?Á?Ö{f™ƒ?¯·Ö"æ?Á?Ö{f™ƒ?ìAÑS¢"Ý?®°¤ÛÇ}a?½ñubîé?®°¤ÛÇ}a?ïYZbÁ(1?§‰§<ª•á?"Ô³§ÚùÜ?§‰§<ª•á3FGL J2338.7+0251@VsI''>ÀK¢±Ä2ÊXÀ:)>ku™àÀ;Çöåv?â#Œò
Æ_@ÛNšÂ¹y@¡u`F²¿ãÜ©""#2¿çuiÛa²¿êÿw(«¿î.'7$¯UNASNonenone?ïÈ¥Í'E½?€V†¥X?{­l]!?€V†¥X?ïFâ"ôûí?£$M6'?—#­`'h?£$M6'?îqi‰ëu?›%µä‹?¨égaH¯Ê?›%µä‹	?蝅Ɓæ?³3C'@?ρ‰èåøf?³3C'@3FGL J2340.7+3847@[	H˒:À6	zû]À:Ž§©&ÕWÀ;Ô¡¹"ËÝ?°áȚS¡ê@
µp%¬âÍ?þ³ŽÀL¶½¿ë>¿0,¶¿í‡¶	U®?ÞXä¾í!g¿ÜB"Š;,ÒUNASNonenone?ïÿý1™?#Q<ZK®A?Ÿ@YÌùú?#Q<ZK®O?ïàÎ	¸?y´ê%70m?oÿù1öGL?y´ê%70m?ï×"ð(‰?sòÿ`S¥?tnû‡ëºô?sòÿ`S©?ïùÀt`˜F?YßQn~²?Hþ.}žç²?YßQn~²3FGL J2343.0-4748@t³Ý)4­ÀPY6z—À9áB-¡úÀ;Ü÷'þL?äzZ3I¥Þ@
%}$p@HVßà¥È¿×°֜•‰¿á$ÂÛ:Š¿ãDvcMq¿æç×FÅ®˜UNASNonenone@?î 3¯©yü?­‰D±ØŽn?¥üÅh`G?­‰D±ØŽm?í¹ä23{?¹[qêMÖ'?²7ÐÞnd'?¹[qêMÖ'?í&aК
?ªËxÑÝTY?¶Ì÷{/¨?ªËxÑÝTZ?ä°Î¼–?µöá·ÙÝ?×üžcΆÕ?µöá·ÙÝ3FGL J2344.9-5647@t¶®}VmÀM/]»œúÀ:éÊ3•YÀ;÷ÂÅ+?Ç<;±'@W½þ¨¼ø@'3ÀvÓ¿â·Î?ŠüÀ¿êOüÁ¥8¿é'Þ¸©÷'¿ïÿååè=UNASNonenone?ïÿ~²às6?èAˁ\°?)£ñ™9W?èAˁ\"?ïȵËTèe?ƒ·Y#_?{¥U‹ÍF?ƒ·Y#_?ïb¦×"Ë?‰¹Y¿S?"«%
&¸?‰¹Y¿R?îG«òË(5?œO{"ˆH?«…@ÓM|¶?œO{"ˆG3FGL J2351.9-7601@s9ÈýŸÓoÀDFÂß
A1À:N2 ä|À;­.ƒ¡	пۗA¹øx'@š÷0£‹á?û›A9†4¿ïÿ⿹z?ïþÌì­<å¿Ñ	Bsíã¿ÜS.¡UNASNonenone?ïÿ‰sAú?	ØÄa™?
£8olá?	ØÄaw?ïéf-z™?qKµ	é?f™â҅h?qKµ	é?ïȤàø?w@«$ž
×?{­ùƒùÍ?w@«$ž
Þ?ïäšÅl¾L?k
¯õN?ke:"A´1?k
¯õN3FGL J2354.0+2722@Zär\=îxÀ@ãÈ}²³FÀ:«ks¡RÀ;þ¢$'–H?Á{µÚv@
œ&"iY
@=ÿg©²¿ìs_ôx¿ÔŠÜŽG׿ǭ€'ú•¿é°6¿UNASNonenone?ïÚZÆ~‰?yµÆwLc?rҜõ@»<?yµÆwLe?ïÌÅbÖ ?‰cY°WQ?yN"ü/È?‰cY°WP?í…w©[/ò?«¥I×	'ð?³ÔBµ&€o?«¥I×	'ð?ï"ã?†µß±"E?ŽÇ< ;œ?†µß±"E3FGL J2354.4-6612@s}¼¾aÐÀH÷'·þ	À:?ïXzÀ<»Üº€š?؆èrÖÈ_@"Ú§
@€å¿ŒóC¿àSžˆÛ¿âæoÇIfb¿èGÇûèÕ¿æ†P´@~UNASNonenone?ê¢ìOMü!?Ç£Hò‰p?ÅtNÂÈ€?Ç£Hò‰q?ï0Ž"qX?§ÏP'Ç>Û?™üÎ/qÕ?§ÏP'Ç>Û?êòW$j¤á?¶kz¢Ö'?Ä6£nUlx?¶kz¢Ö'?êÞÁ½?³ÙbÅn`?Çø"ûݨ?³ÙbÅn`3FGL J2354.8-5245@tº^5?}ÀO#ˆDÀÀ:åw¾}À;¡7qÁ
?ó!–é$e@q"T[!@C}ßÔ¼Z¿è¯S´KæL¿áòUÎÈ¿æQێþØZ¿ïÿóì)$UNASNonenone?æ¿H!–¦?Ï¡֐ž?ҁo¼ÒÄ´?Ï¡֐ž?ëªÖ,2?ËÔҋú"?ÁT§O¿7"?ËÔҋú"?ÜÞ9XÀú?·p6böÄ?áãSŸ'÷?·p6böÄ?ÖÎu´_D?º¥¸³yP?ä˜Å%óP^?º¥¸³yP3FGL J2355.4+6939@]"_®¼@Ž@<œaÊö3À9±a8)<9À;)L$›À»?Ëý5U@
Ò	ÿ2O³@[á ŽÂ?Å%£'·Ôî¿éÞm^°Ã
¿ëšMbx4¿ØôMyÁžUNASNonenone?öwo?cž°v³J?‰•B|â$h?cž°v³J?ï>}6&?¯'CÁ"»Ê?˜0OÙ;=`?¯'CÁ"»É?ì9%%ЪÑ?®ª¸´O^k?¾6ÖÑz©p?®ª¸´O^j?î8xÜý«‡?¡;¼:ª?¬xr0%G?¡;¼:©3FGL J2356.9+6812@]yèPð@'ó!Ë+ãÀ9oÑI3PÀ:ÌÀˆì?ӍŠÛCe¹@âŒQ²z;@
Aߞ`©¿ç÷݆S¿ëš{8Qøh¿çì"2Á¿ä:Ä—UNASNonenone?îVj=L?±œ\Ù¼3?ª™\/~û9?±œ\Ù¼3?î½HÞñ€Y?¶î¨Y¤¿?¤+rçúj?¶î¨Y¤¿?ê"Ó[ëN?³—Єgaì?Å°³ŽRÅ?³—Єgaì?ìS–YC?¨pðĶқ?»…cOm5æ?¨pðĶқ3FGL J2358.5+3827@[ëúÁҝÇÀ7BŒG¡AÀ:0/(âwYÀ;¹‰Úõr¿ØŠ$¾@¨ZéZ¢
@Ÿ?Àà?ïӇ¶–¿âØem~¿â"'«ìW'¿ØÐÁ'°ÁUNASNonenone?ïÿ8˜-×ô? ¬¬T?ìúE•Ó? ¬¬X?ïá ÈZž?xÊ<ˆ"?n_7¥aò0?xÊ<ˆ"?ï•Jnî_?"µ–XmQ?Š­d\h?"µ–XmQ?ïõ	¨gÃ6?P"oc|q˜?Uì¯0y"?P"oc|q™3FGL J2358.6-1809@P¦ ºKÀR¹G"#ÐÀ:SãD8>À;Äꁺ?今ã¦á‰@.ÉA'?ý`ç÷K¿è£p™+pØ¿š¸þ{Õë-¿ÉÁ2\@:¿ââôxQ9GUNASNonenone?ïöDëPé?Vu—ìE?Sv)_Ò,ƒ?Vu—ìF?ïéõ
y@q?pvÄ寔ü?f
ò†¿ŽÛ?pvÄ寔ý?ï}á( L?‡ôژ]ÂÍ?CÚëïÖm?‡ôژ]ÂË?ïE®ÒË?'œ)ï-?ž÷J%¦žv?'œ)ï-3FGL J0002.6+6218@]SRÁmóù¿£äVAÀ8¸4t{ÒßÀ;¿"å­?ÿ®	&šI@ù8ö–Ÿ¿?÷;Q­Fʕ¿Áôˎ´8V¿àõø8Ðø¿çϟA›£,¿ïÿÐ%­õ­UNASNonenone?p5"›>‡å?ˆ4Äèý?ïߔØɂð?ˆ4Äèþ?+Íy.Í?EïrÉ£Ï?ïþC.(n¼?EïrÉ£Î?—I^úNP?"Ó¾-ö…)?ïEµ-}?"Ó¾-ö…&?nº¦MWƒ?\-›"‹Í¤?ïáEY²ì¨?\-›"‹Í£3FGL J0008.5+6853@]ÄOÊB®Ñ@Y»j¤¹ˆÀ9u(>«	À;e£Z»Ð?ýí,€çq@s[T9"?÷ðΑÈêÀ¿Äæ}ß+¿äY_쓀j¿î¾£Fõ¿ïÿbá*¼UNASNonenone?—»ÈLlÊ®?ªŒ¯¹Ê&?ïB!½œ™ª?ªŒ¯¹Ê&?u^7ƒ(Ã?¡¥é¶Y?ïÕÝCù®?¡¥é¶Y?¶/†»PåÅ?¨òâËP¾c?í:(•ãH?¨òâËP¾c?c7FUÐò?Wß]ã‹v`?ïìȹªä/?Wß]ã‹v`3FGL J0008.7+6558@]¦s>»ýr@¤á¼©iÀ9šCã…À;,rÉK8?ý—£FÉ@ÏzÒB@pp€p¨µ¿Ù»0(wÿ¿ëÈvaŽÃÛ¿ãôÄN4Q§¿é쌦t¦úUNASNonenone?Á:±]p¢??¾5 «?ë±S¨£×q?¾5 « ?«ÿœd/ÃÄ?¿&cL°Þ?î@9½Ä?¿&cL°Þ?×qU‰à¦?¸±ÁTkÖ?äGU;þ®?¸±ÁTkÖ?œ¶Dí ò?ŒÓSVœq?ïMß 'ù?ŒÓSVœq3FGL J0039.3+6256@^c {5*"?º$ª.gF‹À9köÔ{À;AŠ[@	.êú	q@;epÈ¿Á'áÙ¬âª?ïý°3Rׂ?yѦ p&ô¿áä³Ä›®¿ïÿü]šK,UNASNonenone?ÕÐ=jáÆ?×~ˆýÌÀ?åáJþ?×~ˆýÌÀ?kþy­æb?ŸéÓƐãÎ?ïäü†R?ŸéÓƐãÌ?¾É´¨ :Ç?°œ¤}³h?ì&Éjëø¨?°œ¤}³g?'2v(bW/?äŠÿ?ïvlN¼íG?äŠÿ3FGL J0212.1+5320@`ݧæšÔÀ•&Rz XÀ8ÊYž×ÇÀ;/`Ëò¥?ýyšóṙ@‡/Kòò¦?öۘð&n)?Lóp*¿Ùë»{–¤¿å¤þLf`¿í—*;:ØUNASNonenone?Mïlœˆ‡?Q›:#ˆîV?ïø»$ØÝ?Q›:#ˆîV?iL¬ªâ®?'Òk"§¬?ïæã³SU?'Òk"§¬?_ò"}?Ke×ÀN8?ï‹þ€5ïÍ?Ke×ÀN=?†a^ÀD*z?sT1ÕÌþ?ï¦z"þïV?sT1ÕÌþ3FGL J0223.6+6204@`¯âXOLn?ñצ_z¹ÛÀ7ò˜ëô°AÀ9àá"-nÎ@»Ð¸ê—¹@
ۚ?±Æ·?ùŽùÕÄm-¿ãÿī웿ہU§Éª{¿ç䌳w¸¿ïÿÖܽ}UNASNonenone?vÖ_¢Ûú?•ÁæÉäã?ïÒS@ºH
?•ÁæÉäã?2£9ÅD9R?KKsߋý_?ïý«˜ÇWy?KKsߋý_?§"ˆÿÊ?œò8´Á"8?îÓ×p_?œò8´Á"8?['¸±ræÇ?Tŝ֕ç?ïò>£§F?Tŝ֕ç3FGL J0225.8+6159@`¸åŸ+©Ò?ñîI9.õ·À8\'jPÀ:ç!éB?úÁ.ãÃ3@¿v×LØv?ü9´¡ÝµÓ?ﻼG¬š¿å"à…Cÿ½¿éäñ
¼¿ï|w@9'.UNASNonenone?ZÇ2»mZÍ?hߝÆwÞî?ïòœf¢IR?hߝÆwÞî?U*hFŠ?o‰˜Üå?ïõj¸pKÝ?o‰˜Üå?§Å¹k'7Š?ŸŒ³¥"ï—?iG܇?ŸŒ³¥"ïš?"îmƒ±5?‡z9<'!Ò?ï_PŒ"âw?‡z9<'!Ò3FGL J0238.0+5237@a[&ÉÀ¯"á¬WâÀ9.ŸÇ±À;pÌ؋Fð?ø4eø­P[@ËÊÒ÷‰9?ý;3L³Œà¿âo5ãå¿àà¼;bµ5¿ä&â涿ïÿéò§}UNASNonenone?—(t-银?žü}Ó»Ú¨?ïF¼^³b?žü}Ó»Ú©?^L­2æ~K?€,U&Ø
I?ïðÙ©fŒÁ?€,U&Ø
J?¹ ¥¸³;?§å%äáé¡?ìËë\Hé™?§å%äáé¡?tAe'R'?{^:ځ'?ï|]ôÓmj?{^:ځ'3FGL J0312.1-0921@gðwÙUqLÀJ.U⊤3À9ùíÓ­'žÀ;ͤ¦©M?ö2´ [)Ç@åYŒä)‹?ñ7ð<ªÒ?ÚDñ«±þ¿ßb{$¹rÓ¿â±ï¿¿ïÿö‰£q#UNASNonenone?á:w™G?Ôwîœa?݋zÍqò?Ôwîœa?ÂpåÛl¿?Íoø	Ph?ëcƉ$Ð?Íoø	Pj?ʛ"Àz9?²ãÕãÀ^?éYáz±?²ãÕãÀ]?»RâOóÑã?®¦ÇZJ:?앣¶…Å?®¦ÇZJ:3FGL J0318.1+0252@fN>ê šªÀEÑG®záÀ9ãpñãºÀ;îu"çZî?ûô`΢:@TÍ¿»í,?Ñc"šë¿Ï¡CS‰6l¿½F$ð'è¿åðÄ4,¿îz]ûͅUNASNonenone?€í³^Ø-P?±_*£ P?ï¼I2"ŸL?±_*£ P?§ï¤(ÈÅç?À6%±Ð1?ss¢?À6%±Ð0?©Ê	€ñ;?£eM,سv?îc_gðí?£eM,سw?›$¨"óB?—Õ¨b½l$?ï&Ú¿#Øe?—Õ¨b½l$3FGL J0332.4+6110@a¤u£KÜ@'h	ԕÀ9¥¦&oÖRÀ;]Æ!·à¬?ö£câ"@Ñ•aüt@>í8}¿Ñ½±•¨¿ê?ùái"?¿ê"oGØÔ¿ïÿ3HE­ÎUNASNonenone?Õºš¬µÁ²?ÊÄòü
y}?å"²©¥'?ÊÄòü
y}?®[W͑‡?¾'/…o?îJƒ&î?¾'/…o?Úß±ÓïL?¶f_›"Ãw?â'w–Z?¶f_›"Ãw?¥ÚÃ*{þ?"¼';€
?î¢SÍ^˜??"¼';€
3FGL J0336.1+7500@`£~=Á@/¼˜¢"ÕÀ9TîDì™À;—éŠrµ?øÀaÖá@,Ó¯*.?øûiÁƒ¿ÓiՒZ9¿Ü0®.ã(•¿ä׆‰ÇiŒ¿ë)'Jê‡UNASNonenone?S¸'‰K¼ò?QxÎkÅ÷?ïö#ì;Z!?QxÎkÅö?'ê1>  q?—kê¦ãê¬?ï´W;}~?—kê¦ãê¬?"`Ç:—æ˜?J¹ÛP"?ï\ùÆ+@Ë?J¹ÛP"?ˆßÜUöÆÏ?r
¡‡?Ž¨$ä?r
¡‡3FGL J0340.4+5302@bXüø
Ã7¿ýí©¼&ŒÀ8ðà9'À;¸h'¹Ñ?üˆY«ìØ@»OÞ9±¨@ÚYO§ˆ¿åÀï7Ë¿îx¿ž)æ¿ïÿ}…^F¿á@ùðÏéëUNASNonenone?á7®âËÙÅ?Ò»W™®?ݐ¢:hLw?Ò»W™®?›á@þ@Øâ?µ}À¨õ?ï õø
ù9?µ}À¨õ?áüîÌø?·µKˆr?ÝÂ#öf?·µKˆr?Œî¬^ò÷?"\_ñ*»º?ïÈEN"4?"\_ñ*»»3FGL J0345.3+3236@d
ʁ˜ñÔÀ1ZbwÄ\¼À9‡G.'º'À;†@@aïß?ùÄ9-D‰@øc^J8?þÑe*|*s¿¸'©öB¨¿éQDɼ*¿êÛåIxøm¿Üš¾ZԍUNASNonenone?éäæÄH–?ÆRäoT·?Èlg˜îݦ?ÆRäoT·?æmëAu`?Õry*Q³»?Ó$)}?Ü?Õry*Q³»?åÁƒ©¿.?¶ŸôTýW–?Ô|ø¬Ã¤?¶ŸôTýW–?ÊêßæX5?À¸¬"íšã?é|EHiò?À¸¬"íšã3FGL J0359.5+5413@bˆLYtæ\?ëæðY|sÀ8nÌ¡-â'À:÷c°©€—?ý3ù;듌@Ÿô§‡C?ük—›<±â¿Öa78·"¿âi‰Ë45+¿æ7ÛÓ>Æ¿ïÿç—åu¡UNASNonenone?v—!ªüû?––a¼åžW?ïÒàѼª?––a¼åžW?)ZB',Cu?Dº{k?ïþj[Öí;?Dº{k?¥;vՓc?Ÿ4Ã^{Æ?î¬NH'¦É?Ÿ4Ã^{Ã?U¨%±pé‡?FdÓþiIn?ïõ+í'G‹?FdÓþiIn3FGL J0426.7+5437@bÛ¾ ºK@ý¸ýâïNÀ8'£A¹ôÀ:¤UÖÌ*@PŠÇn¾ú@•†ø,L?ýæðõvO¿ÌÖùͶ¿ãUº¿ìÝõ›W_¿ïÿDUNASNonenone?"FÔ2-Ux?«w÷¹ó?ïeÉ^n•T?«w÷¹ó?ts—Ç£®ã?›øižÈ²×?ï×Ðp¸¢?›øižÈ²×?¤¡'àd¹Í?ßUuLµ?îµæáù´b?ßUuLµ?xéÑy o?muV'À|?ïÎ,]
Ç¿?muV'À|3FGL J0431.7+3503@d·BZîc À!Ûà›¶ªLÀ9Aû§««À;"n@O{?ö>?Þ½:3@cŸa¯@¿ó£%^‰¿æcb	¬Éo¿éIjX×v¿ãH VÑaÌ¿ïÿÃλ(NUNASNonenone?ßüíx™?ÏòZ:YÕÖ?àõ	C³€?ÏòZ:YÕÖ?®¼/Èåßï?¹y0ƒô†?î=q¢?¹y0ƒô†?ݟWéó©?µá§;ìgu?á0Ts,?µá§;ìgv?¸z"ð5?£†7¨Ö¡?ìü>¯aú?£†7¨Ö 3FGL J0514.6-4406@o/-w1ÅÀA²DêÀ:å	ÚtUÀ;Õâ˜,ž?öýOòÁ`@K&Ðú.@œ¹a`B¿Øda~u%ò¿æñye­¿ý¿ïÿäÙ«Nð?ïÅ7ƒ5:[UNASNonenone?îe5>›%P?²Ž4R6A{?©¬¬Mªü?²Ž4R6A{?ïå]Âî¾¾?{A&ú ›?j¢=A@`?{A&ú š?è=lmeÜÑ?²¦3"±ü?Ï
NJhŒ½?²¦3"±ü?î˜&†y¸ ?³×¾ïœß×?¦}—˜d~?³×¾ïœß×3FGL J0537.0+0957@hiŠ	ÞÀ'(÷À9˜K»ÀÀ;2(@éÈ?÷¸ß9áÎ@ÒåE°a@M:*ž9<¿àNéÐÒk¿ên¹ª¿ì\kñô,@¿ïï–û¦÷HUNASNonenone?ïâF$©ˆ?tC3ËY?m¹ÛVwáº?tC3ËY?î—Fé¥lX?²ëçõñE5?¦‹'e©:?²ëçõñE5?ìäU(àá…?¦`å‡õ­Æ?¸ÝV¸øóÒ?¦`å‡õ­Æ?ìWýâX?®Õéõbž,?½Gpí=?®Õéõbž-3FGL J0539.2-0536@j5®h]·kÀ2›bÇut÷À9@[9âyÝÀ;3whí)d?úAN*…@WMç'@oñ§ÍŽê¿ÄеuÔS»¿ìÝÔ'¿çžr'—ír¿ì'äuNÐaUNASNonenone?'ÕÙ2{,?:ôàAÏ?ï´¨›7ê?:ôàAÎ?‹÷Ð`)ß?žÌ©—<?ï ¾Xƒ?žÌ©—<?Ö`è·gÀì?´ë£™Ôé®?äϋ¤LŠ?´ë£™Ôé®?}[ì¦éó?oFÒç¼2ë?ïÅH'Ö²,?oFÒç¼2ë3FGL J0541.1+3553@e²PÅë1<@¼÷S½À8¹ÈÓC"À:É(çÖz?üӮɺe@{%Y*éŽ?þáñ¿Ò̒…(Ht¿äh³Î¶W¿é¦Îb›x
¿ïÿÃÖȽãUNASNonenone?‰8?›ø3? ûj¤:"?¿? ûj¤:"?CqÙö՞Ñ?T@ž›=?ïû#‰'J™?T@ž›=?¦ubÀ)u¦?Ÿo¤aø ¨?Óýh¦?Ÿo¤aø ¦?bxò|ñœÃ?Ršf@XÓ?ïí‡
ƒc?Ršf@XÓ3FGL J0545.6+6019@câXOLn@/©Á/	ÙÀ9'jËΠÀ;®.Me?øKÂ@¨^ùŠšù?ïdã&€rV?ۇŒ»ÿd¿ÓÂÊ$ú¿ÙWÍW\¿éƒ'ÆSÈUNASNonenone?®''ö'?´#Ç×îªÛ?î×× Ž?´#Ç×îªÛ?Ž"t'N–? ñ¨ÿgœ†?ï‡wî-ºÇ? ñ¨ÿgœ†?ÇHYÈ0¸q?¸±Ð·G?ê-éóÑã?¸±Ð·G?§¶Ê³'¾?–ƒ´°ZÂ?TÎý…?–ƒ´°ZÂ3FGL J0634.1+0424@iáXâe¿ýRøBÀ7Ȗ'•¿À:'zÁg>@Î郑Åe@¿Ê˜@"—hk¿ÓÎÿ‰"ðâ¿è"Dtñf¿ë0yTª§3¿ël›ÿÐZKUNASNonenone?r«L–÷Í?"âU‡Î.?ïÛØ©fÒ?"âU‡Î.?*AMåcH?F?ô£bHç?ïþ[ë!¯š?F?ô£bHç?À'ü½%\?°@QMËà?ëÛ@ж¨ÿ?°@QMËá?Nz‹ çN?EÚýŸ.Ž??ïøa]Æ-?EÚýŸ.Ž?3FGL J0637.5+0418@ið9–ú'è¿ñßX{ÆJÀ8ÅÞSÝͦÀ:¼hA1ùw?ú¶dÙ"@@p"Í@zlnh¿Âۃ«¾οêCnJœ—Œ¿èÌ׫ðV¿ëÚõªµ/UNASNonenone?Ìo¥NÇÑ?Ǘ\£%?èä¸ìN?Ǘ\£%?¨kuY†?´ÀªËLX…?î)Hªg?´ÀªËLX…?Ù@`U¼#N?¸ÿí ƒ=Ž?ã_ÏÕ!îY?¸ÿí ƒ=?É9x é?³N°ÐŽÑs?鱸!ן?³N°ÐŽÑs3FGL J0641.1+1004@iY;%oü@õ¡lèÀ8·àªÐ"ÃÀ:¾­'tâ*?øz0gQ@†IŸ0\i@ªñó—¿âE":{•¼¿çOx1P@E¿ï¹8Î?Ð W3¯tUNASNonenone?àðN^
?Ö>46d?ßÌÍcCæ?Ö>46d?åïWøq½?ԛŠp…<x?ÕÀ!P†?ԛŠp…<x?àú§ºU]Õ?¸pø¶ÝW?Þ
°‹UDV?¸pø¶ÝW?Ý?v®Fg?Ч×ä?¢?á`D¨ÜÌx?Ч×ä?¢3FGL J0704.1-1043@kýHýŸÓoÀ¯"¼
êÀ8ƲœŸÞWÀ:W™?÷Omü]@
µEw•Ü@@-Ëë%¿á¨|&Ö¿èû0•ý‹d¿æì.wпëAßQsUNASNonenone?"64À?"g˧?ï‰ï'»-?"g˧?}‰¨ðÐó?–üè÷c?ïÅÆì®^?–üè÷c?Êzô¾ß'#?¶#•<?éaBÐHx?¶#•<?£m7Ô·å?j"ŸU÷?îÏÙ,'´?j"ŸU÷3FGL J0711.1-1037@làuöý"¿à"5Iè‹À8õLÓi©À:˼zo1ç?ø—h\4ß0@
?Qkr•@¼1ÊèF¿â{ý3¿åÀ´¼Œ¿ì?_®]ÃL¿ïÿh¶«UâUNASNonenone?/de´ûï?žpL‹ˆªá?ï‹Bni,?žpL‹ˆªà?@ ÿn¼°®?Yßê7É)ÿ?ïû÷À$PÔ?Yßê7É*?ýÿÁV£¶?°Bú¿]`?뀪W?°Bú¿]a?…!__N|?sCKþb®?ï«z''Æ?sCKþb®3FGL J0737.2-3233@nÚðEwÙUÀ",Ë:%–À9iÃ9À;6~=ó€–?üÆ~a"Õ<@¶ë+g?üòok²Ù¿ÖQ'[0õŽ¿ä½óñ‡¿ê½?á{¿ïÿÆM¸UNASNonenone?¦Êk/;?¬"‰?î"_yNí?¬"‰?bb"\‡™?'Å;#oHx?ïíÝ£øy?'Å;#oHw?µ¥Z§™fè?ª ØôDË/?íKT«Ó#?ª ØôDË/?†bhˆREL?pÍCºâ:Â?ï¦v]Þ¶ì?pÍCºâ:Â3FGL J0744.1-2523@n*Ûa»û¿æ\°ožôLÀ8u~ÚÑrNÀ;
üaåÎ&?ý
ƒqd]@w@Úæ•÷?ÿ ÛÍp¶¡¿Ú&枰¿å¾3Cû¶¿åþs0Z¿ï‹žw"¤UNASNonenone?†¥í‹	"ü?ªû9ÌÂä?ï¥hIÓÙ°?ªû9ÌÂä?Aà‹Ãñ¡?X*¤E ?ïû¼ÇÝ?X*¤E ?Ä'ÚÆ??±Iè֔hh?êö	Np 9?±Iè֔hh?'Sn?.B²?yŽç"'—ã?ïudŽê?yŽç"'—ã3FGL J0758.6-1451@m>·€4mÆ@?W´ûßÀ9¤¤ü¤*íÀ;"¥]òú?÷3*#êì@
;T˜Þˆ·?÷©æU´èU¿ÑËÁÀÔǿ҄‹rù6¿éªí_Gò¿é¿jœw^UNASNonenone?{J"!ú¬?'÷Áx¨?ïÉk»¼
¨?'÷Áx¨?¡¯H}ø?½Î¯ÕøÐW?îå»ø!?½Î¯ÕøÐW?³±F±QÌö?®17™4,R?í‰×)ÕÆa?®17™4,R?yËâ·–?‰³ÓHëÅ?ï1 ïºD?‰³ÓHëÅ3FGL J0839.6-4133@pRJB®Ñ9?Ô"}Œ.À8†à"&þÀ:šˆŽ¯ZÌ?ýU9Ý@ÜzÛéJ\@™V¸É_°¿hZÀ
¿íø[ª£é¿ëYb…U?¿ïþ/¨0­"UNASNonenone?ŠÐE'äsT?·ê΋"í?é¸n3?·ê΋"ì?Aš,Ý*Ž?XOhó©?ïû½tȵ?XOhó©?Éj–?´"O̔Ó?é¥9=?›?´"O̔Ò?{¢~ò,?mBí+^ل?ïÈ»ɧ?mBí+^ك3FGL J0847.4-4327@pxdZ¬¿—»»`|;À8DmØJ¯À:f]@L÷*?þ(˜¨-G@îþ—@ã?þÁyŽ°\¿´Nµ—<wI¿èg×Û|E©¿ï9EÍÙV?ÁY­Ñ	‰UNASNonenone?ÜaÌçü.?×ê31®ñÛ?áÏýŒé?×ê31®ñÛ?Փ\W«"?ÓÊT?²¿ò?å6QþT*o?ÓÊT?²¿ò?Üìá§ý?º"ü2–™?á‰ò,x?º"ü2–˜?Ïç]iÎñ‰?Ëos	¶ñÏ?è(¥ŒCž?Ëos	¶ñÏ3FGL J0851.4-4244@pvü;Oag?ïÇõݒAáÀ8UÛ¢R¥¿À:iΐò++?õ¿§@f"@
ð¦z'¹W@€'µ¦•¿àÉIY²›@¿ê¶år
3‹¿êØ[#*¿ã{Ìй҅UNASNonenone?¶«.»[·?¼5Ù@i?í*š("ŸJ?¼5Ù@i?¼TWˆ\?ÆóšŸÐ1ü?ìuuü´?ÆóšŸÐ1ü?×=:'5?ºPžõÓö?äsauâ·d?ºPžõÓö?¼Vq£¿èÌ?°RIºL†?ìu1ˈæ?°RIºL†3FGL J0854.8-4503@p™¤ü¤*í¿—tR§¬¬À856£*<À:ŠX;*xz?ýã!°SðB@qíVD?ù-Ö|ùÑ?Ó¬¨Üì!¿Ûɽ£º¿æ4È«ø8¿êc?Dä`'UNASNonenone?NBÁL"cP?J­Ûû—Yu?ïøoO¬÷f?J­Ûû—Yu?8'Ÿ'<™?PiÉü¾ñ?ïüí¬¸m?PiÉü¾ñ?‰í¯?‹ÒXh õ?ï›û³œID?‹ÒXh ò?'ˆý×YÜ?pw¢°ž?﷙Ü¢˜?pw¢°ž3FGL J0855.4-4818@pÂq!«KsÀcҢϣAÀ8gQÌ{n5À:vh@Žf?ÿ‡	½=ä@,/±™Ä@7ÒT¿×H1Ð¥¿êtþÙ»7¿è0 ûHòH¿í¨šêbÆUNASNonenone?^²§{'}'?j_lsê±?ïð¦¬B>Â?j_lsê°?5?JÌi?O¦dªy;N?ïýX¦}3?O¦dªy;N?ăÂap¤³?² •ÍÈüÀ?êßg£ÖÓ?² •ÍÈüÀ?`ÒÓ²Ê1?Tyñ#y·Î?ïï-à,M6?Tyñ#y·Î3FGL J0857.6-4258@p…"ÿCAž?ûP¨È%žÀ8yÊU#HÀ:~ϟåãõ?ø"Íû U@k€´›R¬@ä€ðÖAk?¡
Â0h¿æwúٚn¿ëJ¹4-¿ì'ïHͤ8UNASNonenone?''ó*·0Ë?–à¢HwPÐ?ïkèfªFz?–à¢HwPÐ?¬Y¥[þ?ÀØ'üÉt?î:e®zA?ÀØ'üÉt?¾«™Ðæ[?°:¹ƒ:?ì*ŒÅã4?°:¹ƒ:?»Ú]€¥Ñ/?¨á–¢~–?섴OëEÚ?¨á–¢~–3FGL J0858.6-4357@p";dZ¬?óN~é+0À8;IàâÀ:o²'ž«Q@Ïh5ã@(ب"H?ý$…(0K¿ÐZ"¿æÆĤNT¿îˆ
Aпà.Ý
6ÊBUNASNonenone?Ù¼ÔqGV?×"€ˆ(Ì?ã!•Çs\U?×"€ˆ(Ì?±k`˜OK?ŦRß'¸ý?íғìö?ŦRß'¸ý?ÚÂ5_/\?»ÌÁ²Ì,?âžåP9hR?»ÌÁ²Ì+?š›Â€ÃÄ?–ÞŸù]NÙ?ï/ó!ëùâ?–ÞŸù]NÚ3FGL J0901.6-4700@p½o?Rü&¿Ù@ÝÀ»À8 Eð¥À:OY•?úónçê4'@	Wze¤?ýckw¶¿ä3ˆ"¸$ä¿âš¨Éüý†¿èá›Õ¿ïÿ²§ "ŸUNASNonenone?Ž%Šu?£M
½Õ?ï‡i×Æ)¾?£M
½Õ?^2Pé‡Ú¨?p§üï0ª?ïðæ׋<?p§üï0ª?®¦Ü$%œ?¢-6Måô?îõ'=½¦?¢-6Måô? wü®Í'?'"na'Ü?îø€5&÷?'"na'Ü3FGL J0905.6-4917@pà
å6P¿öÀ³Nv…˜À8†î‰µöÇÀ:¸šs´-@"
¼õ@X‹{ô˜?û?‡ñ\?îê0õ/0^¿é=KR8Üë¿í<Ž"ER"¿ïþvì#1çUNASNonenone?«zŠþz¡?ƈY?ëU!]@aX?ƈY?9Y<¬¶1…?QØ涕‰¶?ïüÔØji:?QØ涕‰¶?ÊÑ˵VŒ?´÷³;äÎ?éK¹Mª]?´÷³;äÏ?zŒª‡;‹?pòç$‹æ?ïÊçöªñ‰?pòç$‹æ3FGL J0906.0-4705@pƖOv`?¸–º›¡À8²äǕUgÀ:}‹–¡—•?ù"Ÿ48@ä@,9—ÑB}?þÆÌÐ}±\?˳–áÈ ¿ê0";¥Œ[¿îøì»Þ±?§gji͛vUNASNonenone?ä/u¿[¥?Ô¼«ÜïL÷?סÛH¶?Ô¼«ÜïL÷?߂¿tÏU?Õ ¶óµ·?à> E˜Uv?Õ ¶óµ·?á›üZ9ž?·ßkË?ÜÈéKŒÅ?·ßkË?ád«>k ?ÍÔù½F•?Ýç6©ƒ)Á?ÍÔù½F•3FGL J0907.0-4802@pӓ ٔ[¿Ú¥¬ÍSŠÀ8Ü滋[éÀ:›#ôÑΔ?úßÐVD/@
©¿³´£?ù2aŸb?ïÿ9†$¿ç×e¿èšg!¢<*¿ïÿ¢å8¿UNASNonenone?À-ý:xˆ?ƕ[p¬¼ß?ëô€¿1aÝ?ƕ[p¬¼ß?Aw;²QNé?WBEB?ïû¢1k¬?WBEB?ĦŸÚ‰¼W?°…ºGàÊV?êÖX	]ê?°…ºGàÊV?àßù[$?âä£;?ï ù5'?âä£:3FGL J0914.5-4736@pÜk;¸<ó?飺º{'qÀ8/·}°/À:žQY•@!!Ðà,Ñ@="àø(@÷(pa'ë¿ÓÜR>™ÌM¿ê"åʬa¿í(åÂŕ¿Ò?ÏezÐxUNASNonenone?ç~LœtÄé?Ê#î#g)V?ÑfÇv.?Ê#î#g)V?ӒØ;›F?Ó¡ovap?æ6"þb2\?Ó¡ovaq?äê¥ÖFm?µ` µH?Ö+À´Ss'?µ` µH?Ȃž§œÖ?Áóø+ÜÞ@?éßzVË?Áóø+ÜÞ@3FGL J0915.8-5110@qÚ{9¿øMzÂ=ý'À8ÞfRDpÀ:ÏÍ"]"?ú•M8`D@õš9ý|Ã@a®‹™%Ö¿ÜzS®'ñ¿í ÙoP"‹¿êOÅóiĕ¿ÎõJ¤mªUNASNonenone	?ÊáI™&ã?ȟhŸR=?éy­™¶H?ȟhŸR=?ѸS]¼¨d?ÑQ•#›?ç#ÖQ!«Î?ÑQ•#›?àn–·7†b?¶¯Ù·Ö5T?ß"ґó;?¶¯Ù·Ö5S?Ém  Ù?ÃÓìdúîS?餻÷ý÷Ê?ÃÓìdúîS3FGL J0933.9-6232@q£Âã>ÿÀ"`úÛÀ9¾ÙÅÔÀ;" ¨ìó´@jl(T@RãKζ¿×ÎR8œ¿Õ™éº]"_?°ïÒq¿á¤"gÑK¿îÊW…*ªVUNASNonenone?¿°)àz;?їö3¥÷0?ì	úÃð½ù?їö3¥÷0?ƒ‰µ¯š²?¦"pS)dh?ï±Ù)A—¹?¦"pS)dh?ª¬í)??«ÜRj!–?î^5?-m?«ÜRj!—?‡)Œ|9\J?‡Íèçe:?ï£YΏ?‡Íèçe:3FGL J0953.7-1510@o~"t¼@=šÿ}úâÀ9Ý8§z¢À;ùõ3c¾?üR:Ð5@
É))D?Û«g𲸭?èz;ì{z¿ÎOo -¿çnS	½C¿ïÿ¬r†§œUNASNonenone?'à2}?›÷ûP¾ä?ï· Ý¿5?›÷ûP¾ä?qx‰†ÜùÙ?'RnD©ß?ïÝìòF?'RnD©à?©dîkf~‡?¡[F ©ÂU?îi±I˜?¡[F ©ÂT?|%'¡b?v‹»é2É?ïÇ´ú½é<?v‹»é2Ê3FGL J0954.8-3948@p݂ýuâ@&ê@1HwhÀ8¹}uv¤¢À;m2˜Ù€9?õËÔ.ÀÝ«@×-xß@a9n'Z¿ãÒ¼"Ëÿ¿èŸ"L±¡¿ä‹»S8óM¿ïÿ¢Gƛ¹UNASNonenone?Þ{´·«Ý¦?Ï]î±¼8?àÂ%¤*.?Ï]î±¼8?—\¾>Ÿ¶?¤ÖÆòq,R?ïE
?¤ÖÆòq,R?Ùo#^šT?¸Ûäq«}p?ãHnP²÷V?¸Ûäq«}p?°"l±{nå?šXpîW™?íïriВ$?šXpîW™3FGL J1002.5-5709@q˜îcŠ	¿÷ƒÆÉ}À8kõœÏ®ÿÀ:O#
KB?öæä‹/s‹@œJ‹¿f]@Â@VÝ1?ÕÆ•^ ¿è	·}œ¿ê1øJ©òW¿êj_«rpUNASNonenone?p'šY(â??}M*"Šë?ïß°ËM®;?}M*"Šë?OéËk´
?kvg¯r¹?ïø%Ù?kvg¯r¸?»_ŒøÉè?¬Ì|‡í¥?ì"®`æÃ?¬Ì|‡í¥?Ç@Ó!-ç?€±JY‰¨î?ïˆâü³{H?€±JY‰¨î3FGL J1013.6-5734@q°ò䎊¿íçù¾ÈR?À8€"¸aÀ:‡dK3'?ü»J}@9[‰"'?ù¯Àéz-?ïÿµÞ¯ßg¿è¹™ÈØ:X¿ëZ®ô¼Å¿äq[ˆ£
rUNASNonenone?ࡶmà#ê?ׂÐü$ý?Þ¼"$?¸+?ׂÐü$ý?€¾vLJ?£þeúaP?ï½ê%¾Ï?£þeúaP?×æ
g¿E\?»™Þ-ï@ì?äùL ]R?»™Þ-ï@ì?¢"	B"Cí?šÅ'UðY?îÖÏkÖ»Á?šÅ'UðY3FGL J1016.5-6034@qÐ=Ć­À	¶	8ÿ%À8¢qȚ8%À:í…AóÀW?ü4_,
@9ΛÙæ@U%o¦+"¿ÕðkhêáF¿íÞ[¦!šã¿è1Xh)'©¿ïþ°ð"g^UNASNonenone?ªOß'òT·?±°fâ4»ä?î[
€Ú´?±°fâ4»å?ñRnÁ"5?¡6U1í¿Y?ï¸:¶Dù°?¡6U1í¿Y?Ñ"L€)w?¹lØ7wi?çznÙ¿ëE?¹lØ7wi?%YD0?}ˇH—Á?ï‹j›îï??}ˇH—À3FGL J1026.2-5730@qÆM@$³>? µÐ±Þ´×À7Èn4'EÀ9þ¦-?ÿ¾‰öct@\è"ÿV?ü6ݲMD¬¿çƒ/NĀš¿Þ8I5[µ¿é®
Í{¦ó¿éE狏–UNASNonenone?PU›;p?KÃ,Öøã ?ï÷õÕ2b~?KÃ,Öøã ?G˜Mþ¿?að.°'?ïúøºl?að.°'?¤Q«8¼P?¢á…sx?îºåOìt;?¢á…sx?'K\Ï¡ß´?vàŸ¸p*¶?ï¶ÒŒÁx?vàŸ¸p*¶3FGL J1035.7-6720@r&@·€4nÀPBÛÀ8`
z­EHÀ;?zF;†@'ð4ÛÕ@Í£ÈDŽŽ?ûôÆ/¿Ä€ó·áó¿àG±èDøX¿æۛÙS²ž¿îCRªò²eUNASNonenone?4I˜™8†š?.yþ"úub?ïývÌìØð?.yþ"úuc?N‹V9èþ«?axH/?ïø]*q…Á?axH/?yþ¢Ÿ•Òö?`XSwRš3?ï̺ÀÔZ?`XSwRš'?a˜mt¤?R0:ñ¶?ïîgþû'‹?R0:ñ¶3FGL J1037.2-6052@qõ"œwškÀT*#¿ùÀ9ûkEÉ8À:õå†6a?ø‡,å'?@
Ââm©Q?þ£ÐqÇîl¿Þ7 <$bO¿ëŒíîÒÓn¿áûÛxê«
¿ïÿÿ¬?…ôUNASNonenone?ÙmܞÒõ¶?ԓºãc?ãI°–…%?ԓºãc?d©³¡<¼Ñ?'ùÆÂ#S?ïëVL^ÃD?'ùÆÂ#S?×á_êLÇ?µí@"Öf@?äPpŠÙ?µí@"Öf@?¤^¼­f…^?"÷3oþÔ~?îº5)—ª?"÷3oþÔ~3FGL J1037.9-5843@qåz–¼¿ÌèöÎþÖ4À8T=;"À:c?J˜ª†?ùhðÊ-
O@
Hy|î"?ü]Bf×пæ1QÚúHA¿äl(
Ôèìl†!Rò¿èJGy€
UNASNonenone?€þS¨pÞ×?‹ZTwf]A?ï¼±^<"?‹ZTwf]A?T¹Cå5ê?o^de#G?ïõ£^
et?o^de#G?Çc‡e:)\?²ƒD¤A'?ê'&±u©?²ƒD¤A'?õÜð?€Úˆ'‰ ¤?ï‹à(Œ?"?€Úˆ'‰ £3FGL J1039.1-5809@qã4¢3œ?ÖuÌ}ɯÀ8ÖmpEã9À:x‹îN?ùžv*úÕ@ü²ÎHøÂ?÷'\ÆÕfú?ï՘KÌîA¿à'ß\¶(4¿æ£% Bb¿ïÿá…ÓiUNASNonenone?œíR0º¬?²Z}
Ž»?ï•nz/ƒ?²Z}
Ž»??QæVÜN?SÝÙÎ+?ïü•Ã5%?SÝÙÎ,?¨±JÚ(P? @-¤'0?îtëR]zÿ? @-¤'0?ˆ>£~"^?}À¦@L¶?ïŸrÇw?}À¦@L¶3FGL J1047.3-6005@r½<64¿ë–eÒ°À8Yóv"Á›À:;°ÂF?øF&ñ}@$	-{8[?ü<|Ã$¿Þ®ØÑñW¿ÄòH'ú¿êÛÞLž` ¿ät+º²²´UNASNonenoneT?®h1»˜o?¢8Zk"˜?ïzŒ¾r#<?¢8Zk"˜?–ï¬>nï?­%÷¼/§¿?ïHêžˆ?­%÷¼/§¿?ς¿vvÙ?¹ÔÂU4U¯?è{Ð"bJ?¹ÔÂU4U®?µ©+Šp]ê?¨í|¶QÕy?íJڎ±ôC?¨í|¶QÕy3FGL J1048.2-5928@qý³Ð|"¶¿Ð¬@$Þ0ÍÀ8Esvð!fÀ:7F°¾yM@…'5yß@¾ÅÍÿý§?úZ¢e›e?ïϯ??¨Y¿Öºèÿ]mÄ¿ëÊÿèƒ¿çoi¡H(}UNASNonenone?À96q'?Ê÷îª?ëñ²|#¿?Ê÷îª?y¦þvj{?¢÷£¶}?ïÌü²+?¢÷£¶}?Ô'œöu?µ a¯m\?åþw¶±"Æ?µ a¯m\?•ÝÅW"¾?IÂfËù?ïQÕC_a?IÂfËú3FGL J1056.7-5853@r	7ޓž®?粓€zä£À82Òò€»|À:°†ˆD݀@ð+Voù@š@QT?ýaÿI ÛB¿Éb_CF¿åÌ<>Ó-¿ëå­X_´é¿ïÿ¡Ïý6UNASNonenone?"èŠØº>?¥2"6'%Y?ï`»©?r/?¥2"6'%Y?&GÏåù?BÑnN"ñÙ?ïþ›ƒ ?BÑnN"ñÙ?µÚÓ(—i??¨ô3µ®Ë?íD¥šíØ?¨ô3µ®Î??Ü2õÒÙ?5/†X®]?ïüy®AF?5/†X®]3FGL J1104.9-6036@r#¹#¢œx¿ØæØ|-xÀ8脹7ÅÀ:~¤™@3gáe¶@l\õyi?øáY÷˜'?ïÿX"ò2¿Ü-vÕ8E¿æ
L|/{n¿ï~@ÝÀºñUNASNonenone?=@ü†r?@+FWv?ïüWào>?@+FWv?0|õùò?J9Û÷ÁÀð?ïýðaN?J9Û÷ÁÀð?*B˜½¤?—†\äR¸?ï~­ë:à?—†\äR¸?iIÛü߂|?`¶µÙï-?ïæ¶$ }?`¶µÙï-3FGL J1112.0-6135@r6^Ý)5¿î¨0 ±»ÏÀ7Ù³×2]À:C6nQs@«húp@Έc¼=?þ#ÉO"¾¿ÑåÅÊ­–¿æôþǛµ¿è]—ÆìÊ¿í£ç?·"UNASNonenone@?W«
w+r%?XR½ƒG?ïô*zÄjG?XR½ƒG?4=€uÁäf?L&ù.£`W?ïýxOñGÄ?L&ù.£`V?´ƒüÚ,/?«פVÊ?ío€dº}?«פVÊ?n¹s"mÞ?aŸžc«ì?ïáFŒk'!?aŸžc«ì3FGL J1119.9-2204@qGƒ[Õì@B†6`åÀ8Ώљ»(À;™tÆ{yô@$7÷E¨@Œgƒò¾N?ö
óxˆ'¿¥øV9]¿ß,âP–¿è Âb(‹¿ïÿê#¨YYUNASNonenone?œÅÌÏ
‰?£"']Î[?ï!љ‡¬?£"']Î[?uÍUÄÙJ˜?ˆì¥'Ýò?ïÔeTvMj?ˆì¥'Ýò?½'-¨­g?®9æiŒ?ìMº\jêS?®9æi?m<x,Z"?csXæ4?ïâÇӥm?csXæ53FGL J1120.6+0713@oqÝDU@NW´NPÅëÀ9ÒñÑsûÀ;åû¤P¬Á?úèE‰L‰@þEjÃB_?ñ›±‰¥ZÃ?ïKT
¡Í¿Þ~G˓R¿äH§Á¥|Q¿îÃËV€bUNASNonenone?°6èÙ>ä÷?¶«֏¶?íù"äØ#a?¶«֏¶?º½(WUo?Ç¡ˆqÆi?ì¨\zõR?Ç¡ˆqÆi?Ê&¿¦…®?·j×ÔØ+?évPy"?·j×ÔØ+?Á0éyèÓ?°û¡lò>{?ë³Å¡ºÅË?°û¡lò>{3FGL J1128.6-5434@r0˜ñ/@z	Ì1œZÀ9eDܨâãÀ;cÚTtÌ[?÷9ÞóëË@
M¢÷Œ¿@
l…E¤¥¿á×i'òÛw¿ë+fiþ¿ïØڌï¿ïÂ
H½ÞóUNASNonenone?ņFP"¨?È
ŽFöÑ?êž®k÷V?È
ŽFöÑ?Ēô'SÏ?Ð;‹šb,l?êÛBßk8?Ð;‹šb,l?Ú`¥fV ?¼/¨+i0?âÏ­9LÔ°?¼/¨+i1?»:U"Jc?‡ð:ÚL?®×?‡ð:ÚL3FGL J1128.7-6232@rYŸ±¿òÓe7'=…À8º5À¬-À:¶î#;n?ûó"vøYî@|CÐd[õ?ù!֙Õ(¼?ïô`9¦"Õ¿è:5+Âå¿êg…î
‡¿åáe<3¦ºUNASNonenone?³þàûzœ?º»HÆôe¸?í€#à½-?º»HÆôe¸?wcWÃ.™
?¢YjÛsð?ïÑ9Py¢Î?¢YjÛsð?Ôn¿V)?¼QÊUëx<?åÈù @Tì?¼QÊUëx;?žnY.'¤?'ÜY£Rè"?ïÅ6‹j?'ÜY£Rè"3FGL J1208.4-6239@r ]'ýuâ¿É¿{*˜°À8ô!-wÀ:	÷;5`4?üJ5XQ@©·6ì%?ö̼†®…d?éòz1Ìß¿ÖÀ}xü–¿å®€Rî¿í§õ'ùoUNASNonenone?ZýÂg§ç˜?c'Öý¤s|?ïòÌ,?c'Öý¤s|?dÆ·«²Mß?{NlkÐõ?ïë9HTM²?{NlkÐö?™W·"ÀaÓ?›÷f]êM?ï5BCYüò?›÷f]êN?©H˄?œÆ)n#õ–?îgësG¿?œÆ)n#õ–3FGL J1225.9+2953@g$ÞÊl @Tðñ¾ôœõÀ9wÒ4jkÀ;¨Öí·ÿ?úOó«³Í@>¥"8äù?óJCðð™?ÒïXæ© U¿àW¼ãÜÄù¿×UXÂ8õ¿ì'ŠyÉ£*UNASNonenone?"€ÊÁmž?™u…"µU?ïcù©÷Œ"?™u…"µU?Ê`äºêÊ­?ÓÙe‡EÍß?égÆÑEMU?ÓÙe‡EÍß?ÅÍׅ"%?°@‹HCØ?ꌊ·\¶?°@‹HCØ?¸M¢Ø£% ?±Ä릌?ìöK¤ë›\?±Ä릌3FGL J1231.6-5113@r¼Aò×s@'»%}À9fƒÂ—ÀÀ;uëGWL?ûšÄÒW{<@ĂLuúX@ó¡­k¿Õ:æÄ*ù¿èAܕ†~N¿ï礉·¤G¿ïØ¡—>ö`UNASNonenone?ºÃ%Iz¨Ë?ċËØ[X€?짛VЪç?ċËØ[X?zRç»X?–˜©bŸ°ç?ïË[çÚ0‰?–˜©bŸ°ç?Ô¢•pà?·Ýúïÿ?宵Gÿô?·Ýúïÿ?v¢''s"®?j¦/W§î?ïÒºúÛØ?j¦/W§í3FGL J1306.4-6043@sKœ¶"Œ@±]''À8xÅ
»ªÀ:¶…F%~??ÿƒ>ùºì{@™;³4uS?õrjùs¿º¯&&bóÉ¿Ößë}ù¿àì6GöÊÞ¿ësiø¥²UNASNonenone?mîlh/fµ?s;ð"qæ?ïâ"—Й?s;ð"qæ?4#Ç{5,?L¶x=zR?ïý{‡™Z?L¶x=zR?¥€ŽJL' ? =ѵV?î§÷[6Ö? =ѵU?`.$ÍNA?RÊ(Oøâw?ïïÑÛ2±¾?RÊ(Oøâw3FGL J1317.6-6315@sñ¾ôœõ¿á3Ïp;ÑÀ8?M«"}©À:g"©GŒ‡?ù9í|o½'@a'ÇMµ?ûJ)©ò'>?ïêu^üº¦¿ã^,æ#é¿è&lX÷F¿îgùt±¾æUNASNonenone?Sv-íu?Vï&(¸¶?ïöDþsé
?Vï&(¸¶?K"ý¾u?a›G^?§?ïùÿ€b?a›G^?§?Ž7(šdÑ?‰¬!f»¢?ï‡#]–o¨?‰¬!f»¢?›pK7Bh?‹Ä-ªÇ®?ï$e¦Eí?‹Ä-ªÇ®3FGL J1329.8-6109@s8ҝÇ%Ä?õÕ`IôÀ8ÔG'‡|À:€ŠÔÚ¸?øBw÷]o@Åßó›?÷pµµ.£¿Gctö/¿ÝÓÙ"à¿âõ‡›D¿î¼P3°AãUNASNonenone?]²v@F·;?X¸»8'ä?ïñ&Äßܤ?X¸»8'å?ƒÙ³ñ]g'?£økòã?ﰙ0:Šd?£økòã?•¼ž×ÿ\? Ɂ×Â??ïR	@? Ɂ×Â??¿æËï(©?ªw×oíT?ì&ì?ªw×oíT3FGL J1350.4-6224@s[ZîcŠ¿Ôy4¿zSÙÀ8i1ÈÏè
À:sî,ëñ?ý"£'–Æ@B%±ŽX?çµçF[ë?ïúT\ü¿Ñ¿•_V¿â"°õ·¿ïÿò|ðÒ¢UNASNonenone?·"X‡z<?Ä^UÕ[6C?í
tïp¸?Ä^UÕ[6C?S'ӓó€Æ?q'馷v?ïöl6??q'馷v?­kPSÜ<?¢¬%²'©6?î)JúÂ?<?¢¬%²'©5? &¤¯Oz?"A
¢^U?îý•µ?"A
¢^U3FGL J1358.5-6025@sr	ԕ+?õè|4gÀ7䐴Ê!À:Sýå¶?ûI"dvL8@Éf<J7@Çþ†Ù#¿ÒVƒ¾Õ­
¿ä˜Ñ1$T¿è'&›É¿ï-9†ßW¿UNASNonenone?]ꑙ®ùª?d_1~ Ï?ïñ
·3(ƒ?d_1~ Ï?Ge¬[Î?`9+müxÊ?ïú9¦"é?`9+müxÊ?¥ªw÷ò'®? bwK€?î¥X€€×Õ? bwK€?†Ç×?u*e·!?0?ï¤áË·¨¤?u*e·!?03FGL J1405.4-6119@s{!Bp?ҕa¼­žÀ7Ґ[,À9Ëp£×
=?ÿñ´â@BüŒX'?þ_ÛÛ£
¿Ó‹
9ÏYš¿ä]ï֫⋿çvº 5¦;¿ç"vµû
^UNASNonenone?\R²ÁS;Û?m±½É­?ïñÖ¦ŸVb?m±½É­?4Õq2U?Lò£Í^?ïýeQÙ¿?Lò£Í^?Á"H´>¡?³/Æ)'?ëšíÒðW½?³/Æ)"?miÿ9[O`?bß ƒSÀo?ïâ–Ƥ°?bß ƒSÀo3FGL J1411.8-5743@s˜•1ã¨@èX¡ÅgÀ8õil«$À;Î70ö?øº¢OÎ@'9"áV@áÈ¿Ì߿ŧä•o¿ë·Ö¡-¿æ[8'R3¿é†¤9ä/óUNASNonenone?¶k?ÏÁ±Ù?³ˆÊ̯?í2˜ÉÅ?³ˆÊÌ®?·£Ï¹Ç—H?Ãßäs?U†?í†Ç
?Ãßäs?U†?Öz'Íå?ò?·†NiÈ©{?侙
`?·†NiÈ©z?¬w¯­â†î?–7‹Ý"?‰?î8…!ב?–7‹Ý"?‰3FGL J1412.3-6635@sm¹à`þHÀê°]*}'À9†ŽVox^À;@ï›2÷?÷U¸ìp+6@ò©nοÁ?ú2IÂ°¿Ýy¶rËØ¿âi·š›¿åœ0õì*á¿ïÿéåèUNASNonenone?ª@=ÃKä?³ísZ¨÷2?î[ü#ËAÁ?³ísZ¨÷2?•ÿïn×Mn?³wv);a	?ïP"‰E–?³wv);a	?½H,?ªA*V¦?ìVý],Z?ªA*V¥?«ç>h‹I?šÈ³pNGz?îAŒ~§L?šÈ³pNGy3FGL J1447.3-5800@sÜï4Ö¡b?÷®ITèRÀ7ÿö¶«"XÀ:…Ћž.T?÷¢!Ódk@'
t­@Ýë´½·¿ã€ÌÝØ|¿éy<˜üT"¿ëøcb"¹z¿ê¹ËÌ$cëUNASNonenone?™©gEĤj?¡<.ҍS?ï2´ÅÑÚÜ?¡<.ҍS?'AeóÊ?§}O²;åU?﷚úh3Ý?§}O²;åU?Å%M¡/æ¶?¹‡óÙnãa?궬—´R?¹‡óÙnã`?šäY¥ËR?‰¹¸TϦ?ï(ßU2Ѧ?‰¹¸TϦ3FGL J1456.7-6046@sÚVlô!¿ø˜}õÏ$–À8I)B©DÀ:.^¸<?ûCç@ìY@"óoMì@'åÆmã¿Ãö'àªáQ¿ë^}õàS¿ì"f›YQ¿ì17î-ð~UNASNonenone?e:ß
¿>†?p"ý;š¾O?ïêÅ õ@Â?p"ý;š¾O?"C­ÍóN?¢Ih"?ï®ñKðÈ2?¢Ih"?ÄÖ/¿Rp¶?³HT'…?êÊt+cÓ?³HT'†?•Ž×¤û'?‹Y¢$ÏÊã?ïS‰BØ'+?‹Y¢$ÏÊã3FGL J1503.5-5801@sûX£/D'?Þ7_úfŽÀ8–—†™ãÀ:5œBÁE°?ù§œSÞ#Œ@Øٗ
ž?þH»eqHî¿Úù> #Ìc¿æòn-@f¿æ¯'ùš¾»¿îڌ{×oqUNASNonenone?›þ\ºY?£Ÿ™ó~œð?ï'ð
-7?£Ÿ™ó~œð?ƒPÞè@çÔ?•åB%šR ?ï²¼"^üa?•åB%šR ?É^ð£?´'ù*?é¨CÏ`?´'ù*?»$sÐ<½l?ªY`ð%?ì›q…øhR?ªY`ð&3FGL J1528.3-5836@t"»â.]á¿û"à¢l¦òÀ9~e`¬éÀ;_Þ+™á¾?ý}©^2»>@ë.QL#¿ã–/—ÐÊ;¿Ö؎ŠO'R¿¤ëÄüÍ/C¿æ!ڛB¿ïÿÇí%CUNASNonenone?ÚñÆ^¾–?ÚÝ(f˜¶à?âõ‡Р´?ÚÝ(f˜¶ß?Œ¸;ƒËÍ?²:¥^«­®?ðÑ?²:¥^«­®?Æa´*(ê?µïFgSŠ?êg'õuÅ}?µïFgSŠ?žÖ›‡õ^?¡pLvvæ°?ï	K#ÀWö?¡pLvvæ°3FGL J1539.2-3324@u,%ãS÷Ï@1ˆÁDŽPÀ9.èŒEôÀ;š^x[[p@(Ò·rrŽ@;«Ò(+¿ó…¦÷ú"?ïþ°Q/â?ç¡eº]Î+¿Ü>S"ø䔿í‰ÕB€òÈUNASNonenone?Í¥I=Õ?×öêÓÜ,?薼-½ð‹?×öêÓÜ+?±ïËvx?Ëf¡ï&¾õ?íÂ&'<Ñ?Ëf¡ï&¾ô?¼Ÿ5%x?°Î3/¥J?ì|]l[R?°Î3/¥K?"&k@¤.S?Š®Ýi†?È?ï¯fRýoH?Š®Ýi†?È3FGL J1543.5-0244@K¯'9*Ä@Cs7âÅ\–À9ÀÁœ¬tÀ;¬U^f?ö|»WYƒ)@±¦˜/·(?þG;N	οҙÎeܱO¿âÞÓüýþ¿ëù+'Lm¿ïÿ¨×¥ýUNASNonenone?ÔQÏtnÍ?Êð¸£|8?å×EÈöš?Êð¸£|8?Äö­²e?ƛOvŒ&Ú?êÂxԓy'?ƛOvŒ&Ù?Ñ*ÉÍ*ù?¶wÈh¾<5?çj›jƒ?¶wÈh¾<5?ºfzq°s´?¥Ç£J•+É?ì³0±Éñ‰?¥Ç£J•+È3FGL J1552.8-5330@t]$žDú?ÓkM
ìÓÀ7å-c™ÑÀ9ùt,!Æú?ÿþnÞ,µ@´Š­B˜×?óÕ7‡€½U?ïÿŠºZH¿Û+4*©ø¿ã¯wuhž
¿ïò]΃AUNASNonenone@?j箧;;;?'ÿw`8EÔ?ïåQXÄÅ?'ÿw`8EÔ?8ºüCô2J?RŽ:*M?ïüè wy?RŽ:*M?¡gn~8ah?¢@š…`Y×?îé‰yé?¢@š…`YÙ?~¡|C ]¸?t@ýþ'Š~?ï½y¿E?t@ýþ'Š~3FGL J1557.0-4225@túB¤TÞ@ ¹mmÁ¤{À8ÔÔ{øÀ;
Ìhù¾?÷ÇV%{˜@þý~Ԝ@HåY‹Œ'¿ä Ä+q%¿ë[4aº
¿èM9Þaä¿ïÿT,ÉFUNASNonenone?˨0—Ë/)?Å#ý¢ 	?éóÚ
45?Å#ý¢ 	?²	Ï{?Âfý­Z¹?í¾Æ°ž??Âfý­Z¹?ØÍk.õ¡ª?¼'
†Û?ã™Jh…/+?¼'
†Ú?›ñ"çVì?…':â>?ï'vèÅH?…':â>3FGL J1601.9+2306@CDÙê¦Ò@Gx($xÀ:_ñ÷ÿ€~À<@žReþb?÷6(¦I€@ÎÝћ¿¿Ûäúr™Çß¿èÅ&õ?Îkƒb0ÝÕ¿çD uRº¿ïûõú KUNASNonenone?Û××Sï?Û¸^í@ËÃ?â~V}?Û¸^í@ËÂ?ŸWª'W?»µS;Ãþ?ïGŠ«uG?»µS;Ãþ?Æø¨h	w%?ºÅà‹HÆ?êAÕåý¢6?ºÅà‹HÆ?¤2Hû^hÆ?©-)ã
Dn?î¼ÛpJu?©-)ã
Dn3FGL J1622.9-5004@tÛMüã¿Ñíþ`BµÝÀ7nœwškQÀ9ïÇßþù@ T¬)¿@ö¡æÅ~?ò¬œ2Ñ
¤?ïþ¼ö\í¿ÓfIyàZ¿á">‡ïø¿èªs£UNASNonenone?Ÿ~™	¤L¸?£ÃèkžÂ?ï7²Ý›?£ÃèkžÂ?U‹´+ –?p
Žòz´€?ïõtº%ê/?p
Žòz´€?Î<½6/?´ÎÐp²3?èpв~t;?´ÎÐp²3?™V&`[µö?ŸX3¥d
?ï5NÌý"P?ŸX3¥d
3FGL J1624.1-4700@u•¿ðEx?û«>ËÌÀ7öك"t—À:ƒèäö@ÏM%²—@eý€ò"@¬.õ5÷‰¿àHÅ]0¡w¿î6ý'½\l¿àY®eƒ'¿ê:"39EúUNASNonenone?ǯ£nӔ¶?ÄûúH²Â?ê$KÓ?ÄûúH²Â?ŠŒ÷È*?«0¸Õb;Þ?ï•Íø ßÇ?«0¸Õb;ß?Ðz±½tg?µVS֚ü ?ç§!EÌz?µVS֚ü ?Œ¢c}¦?…§}£x?ïvr	g˜?…§}£x3FGL J1624.2-4041@uI&Á½¥@'x³puÀ8f­VœÀ:Â(4Òo¤?ÿØþÑ×£•@l%y6LÃ?õep•x?—{^èV¿à^]eX@Ö¿å…2ƞ¿î±Èe› "UNASNonenone?Diý=?>™|ôf?ïúå»ù¼A?>™|ôf?x烑ès?£	ÂÂçt?ïÎ0øÜ/?£	ÂÂçt?{YåÕOêZ?r–°——¤Ç?ïÉL4U`+?r–°——¤Ç?'Q=ï?n'ó…Çh??ïÀÛç]ӄ?n'ó…Çh?3FGL J1625.1-0021@+Âþ`Ï6@?Özúr!†À8¸@ƒ}ÎbÀ;ež8dË\@+ÐïòÝ@ô?ß n?é…ìï_§c¿ËUO
¿½­mÌaB¿äãaó Yοï¯8gOšUNASNonenone?5+z^EÌV?+mZ©‡²q?ïýZ´7F?+mZ©‡²q?oªñá–ú?ƒ0‰
³?ïàUi?ƒ0‰
³?"»ÝPLð9?"[gÅLª?ïb!}˜~?"[gÅL§?=øši$rP?4³¥m«ð?ïü@ì²Ûq?4³¥m«ð3FGL J1626.3-4406@u%øa¦
E@ْ]e5åÀ8®•Í\>ÅÀ:lñý2Æ?÷Q¾SEÎ@
lÞÃo¾@(qrÂÀ?à¾ñ¢šO¿îÍfØ°7¿¹4xJZm¿ïÿ¬Lh}1UNASNonenone
?Ł\W•)?Í æüæÍì?꾨ê¶?Í æüæÍì?ÔèÂ!p¸?ÖA◜b?勞ïGö%?ÖA◜b?ÕÍN§ë¼?´‰èSt‹?åX¬wŠ"?´‰èSt‹?ÑäŸMª…à?Å;Uôf/‹?ç
°Y*½?Å;Uôf/‹3FGL J1641.5-5319@tԻ¹M"Àh†
 zÀ8·Â,_Ú[À:Òð§h[?ü–$,?Ö@ªJkÞö?ÿā6÷8¿å`ý6ÞÀ¿â$¿²²ð-¿ë¥ÄD_w׿ïÿ†™v'UNASNonenone?‡ýæ&Æü?'ðf›Ö•?ï g·dä?'ðf›Ö•?{Ö\dqv?š½]'F×?ïÈSG7ã?š½]'FÖ?´T³Ê œ?¤ý:²X{Ÿ?íui†«ì?¤ý:²X{ ?•»‹²Ç½ö?†Y<ŠÔ~e?ïR#¢iÂ?†Y<ŠÔ~e3FGL J1643.6-5002@tÿ÷—|À"¬_nû`À8Ì£²!OÜÀ:©>Ò£¦?û:"ˆ¹@tš{ìµu@ƒ@;ÚL¿ÐväÎKR¿æ
vrf鈿ï4·¬¡€¿ÍˆV8¤iàUNASNonenone?álGDy^?Ößû£×Z˜?Ý'pßw
C?Ößû£×Z˜?àœª}c˅?×˖ßK*P?ÞÆ«8hö?×˖ßK*P?ßÐ0qe/?¹0Uøb1?àçÇ|Íh?¹0Uøb1?ĒÙÕ©W´?Âe¶WþS?êÛIŠ•ª?Âe¶WþT3FGL J1645.7-2149@vay=Ùc@.D£çÑ5À9'E«Û»}À;om¿öûu?úôõj¥»;@ç²ãA®K?ðž)¶²¯¿Ç¯¾(''¿àuIó`Â¿éï¦Ä$‡Ÿ¿ï¤Ñ¦ÙÑ¡UNASNonenone?>¬Ç'òÛÇ?:È£äkh?ïü*g
Á¤?:È£äki?yåT´áÌ^?‹4Ò rL?ïÌ5V–<f?‹4Ò rL?¢ ÎÉ,,ÿ?™Ú¬‡òf?îÕóm=0?™Ú¬‡òf?}hçË?rf Ï.T'?ïÅ/à1ØÞ?rf Ï.T'3FGL J1650.3-4600@u<Ãa@O¿îxd•«ÎPÀ7"`X/kþÀ9ÄÉ«?þýøKU¾Î@â¬2#?øwïzÌ¥?Ðs"k(±¿¿àÜù6¦ôæ¿åïólìõ¿ì
ŽDUNASNonenone?4=V̕¢m?,@ÐR^Q?ïýxU&mL?,@ÐR^P?PN[/ž²?ež<Ӊѽ?ï÷ØÒ?h1?ež<Ӊѽ?r»U"3Ù%?X›ød ?ïډT٘N?X›ød?•
Üy_è‡?‹ãñyLhÜ?ïW©5»?‹ãñyLhÜ3FGL J1652.8-4351@u[¼w¯d?·‹Y:À8]–
˜à6À:_yv
£W?úÎMÖL¨O@«}ůÞ?Õ	u…ÏI?ïÿî]ýG¿²§3zʯ8¿äòç
2*¿ë¡ ۆ'ÆUNASNonenone?—¸
"ìhš?±c6n`º?ïB?"Øœº?±c6n`º?‹ä¼û³?±iåtGªõ?ïoá™?±iåtGªö?­ñé•åo–?ªŽ¤ôð?î áf¡©?ªŽ¤ôñ?²ª
Z×)Ë?ªŸ<ˆÿü?íª¾T¥Ç?ªŸ<ˆÿü3FGL J1653.6-0158@0ž=æœo@8ì´Zåÿ¤À8õŽŒöÀ;†"éß,@Gú~¶¿D@þ4x؄?ý'úƒ"I¤¿×'^:â˜Ö¿âFúR
‹P¿å?çx8­¿ïÊ8&¦Ì¢UNASNonenone?Z'7Ä¡.?V;V­
³?ïò¸6ä°?V;V­
³ ?sI˜NÄ?€YpÐGC‡?ïÙlÏbwÝ?€YpÐGCˆ?ˆ½úç=ã7?‡®ßU&'A?ïcs?‡®ßU&'D?kv|ûe8Ò?Xjõ™®Y?ï䉃šÈ?Xjõ™®Y3FGL J1654.3-4907@u!ÀD(NÀ°WK@pÀ9»Z´|À:Û¾	»j¥?úp¥+H-@\fA''–@×B¤•K+¿äëÌÂ:øy¿æÓ*ð6ð¿êË×qÿå¿îµN»-UNASNonenone	?ë+(·J?'ÅÜÔÆL?ïÀ(å©®'?'ÅÜÔÆL?‹Šp}Kx?§òWVJÊÛ?ï'Ö>¾Ñ?§òWVJÊÛ?ÎÛd>ãcÅ?µ4Gßy?èI&ðG'?µ4Gßy?"Ÿop?€Õ‰y5~€?ïgw¹ë…?€Õ‰y5~€3FGL J1702.8-5656@tÆ]cˆe•À"}DUGZÀ8*ºŸ£ŸÀ;'8|HP?ýŒBn@K}u ¾g@ûaŽ»D9¿ßÔâJbyÈ¿å2'¤¬¼¿èSXpj²b¿é®!/>uËUNASNonenone?¸šh¶ó_®?³û‡¦f¡|?ìì²é!"
?³û‡¦f¡|?{daÎ[ y?‰~®¢€…?ïÉ7<cI¾?‰~®¢€…?ÑР"!zy?¸Y…‰V?ç¯îïBÄ?¸Y…‰U?™Ÿû!z"ò?Š,lµ'6?ï3&ô+`?Š,lµ'63FGL J1727.7-2637@v}T!ÀD(@FœÒ3>À8–ØÐN,À:¶[Ëر?ýdÕ÷ú@ A]òz@k°ªØ0X¿àëïhò̀¿éýç"fh"¿ï†¾7U#?¿ïø0ðŽjUNASNonenone?ԘÀ"­Sð?Õ=•t\?峟½©V?Õ=•t\?˜9úUøÅ?²çèUº?ï>0/ÍP:?²çèUº?ÏQ¶pÖÙß?¹z EÈœ?è+'cÊIˆ?¹z EÈ›?}Ö¯pntJ?n£fƒ,N?ïÄR¡#?n£fƒ,N3FGL J1729.7-2408@P÷[ìá@AêÝYÀ8z«°óRsÀ:ÀÒ£¦bÖ?÷¦Zøt"@iÀÆY@8@üÞßHûG¿×Ù^ˬ¿ê…..€`¿ë±N¥®ö¿å·nðèNÍUNASNonenone?ÁDaV‡®?Á!†ÏãGã?ë®çª^y?Á!†ÏãGã?Þø®ýº?×\… !§÷?àƒñ¨ø#?×\… !§÷?Ý(í*/"¼?¹Éü
L?ák‰jèn¢?¹Éü
L?°O:¤\—Æ? z©«T'É?íö«tm? z©«T'È3FGL J1729.9-0859@.oõHìÙ@+&æS†ÒÀ9Bs9³õÀ;9/bÄw?úþø–T?È@
ÜTÎczÏ@må|ñî¿Øê(@§t¿ì6'üDK¿ïÿ´h¤ž?ïð¦ä/êÔUNASNonenone	?áÝ·ƒ8§…?ÒÿYó¥R#?ÜDùŽ°÷?ÒÿYó¥R#?í¶AáÔş?Ç}Ͳò8Ó?²MðñYÓ?Ç}Ͳò8Ô?åE¨ÿê]?´
Ý<9?Õuà®+F?´
Ý<9?ßGó¶—ù?Õ:ÎAc|?à\$´p"?Õ:ÎAc|3FGL J1730.6-0357@3ͽ@gÏ@/în"ŠzÀ9Ä斢nTÀ;gæ…·?øðMÈà¯@3·«þK?ߣK¥¤¿Ú–ú©T?¶k\€š«N¿â_lµñû¿îT'BÙiUNASNonenone?m`Ôàɼ?nqølÀã"?ïâŸ+à6?nqølÀã"?|0~1Ãú\?ñM:¯å?ïǟœx?ñM:¯å?§ì¹ë±@K?ÂD…œ?î4aDëû?ÂD…œ?†eK4°?¦g•bà™?茶jÓã-?¦g•bà™3FGL J1734.7-2930@vd*Ã") ?û6«Þ?»ØÀ8•—Œy§À:zŠÊɽN?ù¼Á"Šf @¡œò¿?ö>À?°uñWrb¿åýu·¿ç$ù³yƒh¿å¶$ÿ‹2pUNASNonenone?Ø[g;ó[¼?Ë©òR?ãÒLbR"?Ë©òR?׺ûÊ"Bi?Õl­³?ä"'îÞË?Õl­³?â˜¬Ðÿ?·©+­¥DA?ÛæϦ^?·©+­¥DA?ÔធC¥?Àåùь?å0¶Þs.?Àåùь3FGL J1736.0-2701?àWà[õÊ@iÏ!:ã+À8¼°³ ¬À:œ÷½;_R?ù®WÙÛ©	@
1î¯ËŠ-?ùmª*5ˆ£?åËñ»C¸g¿ç¼—šˆNe¿åuµ}"š¿ïÿáïôšUNASNonenone?·žÁq3þ¢?Á®}Ð3=ö?í'Ñـ,?Á®}Ð3=ö?`‹6þÍë?p3–d/gI?ïïtÉ2?p3–d/gI?Ç¢Züf?±^—ªz…N?ê8W_©@æ?±^—ªz…N?"^g>ÕT?")·z¾±?ïeÆ	W†?")·z¾°3FGL J1736.5-2839@vr÷eýŠÛ?ýn'«?´KÀ8—cW¾,÷À:´²G^?þqõ0K¦@/° ?ò`àëgÿã˜YþyC¿ÛΆXÒ²¿ïÿñÉ 6[?ïöúNKx¶UNASNonenone?âŸÖÕo,F?ÔÔKO@\Å?ÚÀRU!§v?ÔÔKO@\Å?èÀv.‡VÑ?҄UÇÈ-?Ìþ'E⤾?҄UÇÈ-?ày¸³k ?µ‹åNR??ßŽ™(¾þ?µ‹åNR@?ç°{IÌp'?Ð?*¿Â:?П	lgÛ?Ð?*¿Â:3FGL J1737.9-2511@B¡µÇ͊@~HÀc1þÀ8O#—´½À:ÙXÌIð?ý
Ä<°`@ªNò]U@ÔäÁ5>ü¿áð²Q˜Æ¿é8¢=­	¹¿ì5Ì>ïÿ>"Ó—uUNASNonenone?ÑH(Í=¥Û?ÊBö$ø'?ç[ë™a-?ÊBö$ø'?"`†;®Z'?«1뎙™®?ï\ûÎ"+?«1뎙™­?Ò<œ?‡yd?ºaëx<?æá±à<CN?ºaëx<?'Y̹dE!?€¤Ài"?ïm1š4Ý×?€¤Ài"3FGL J1740.5-2843@vy>Õ(?ñVWûi˜À7kŽ#CÑçÀ9Ó=¶CôL?ùIA<‹@³¼Òì™@ir©´¿Ï…Xþ㏠¿ç»³Ï½¼¿é|ç´Q"T¿ènÜ*ÝUNASNonenone?cq°ÚXå?tž	­¨n†?ïìíŽO%¨?tž	­¨n†?vêãÌ5	b?¡i™ãhÜ?ïÒ*8g•î?¡i™ãhÝ?»ë£úY¿?±Û¿|ð2[?삋ž`´É?±Û¿|ð2\?š=ÛnÿQT?ŽÓiH¦TË?ï.$ˆu?ŽÓiH¦TË3FGL J1740.5-2726?妟ê$Ì?û»èÿ2z§À7ù/‡­À:3µ«HÇ?ý§7è¥@1	½@ÛçF÷¿Ùv.ü¨î²¿è{+½ÑÞ¿ê'ôRLÔ¿ïÿ›o÷M™UNASNonenone?"¦j…ÌJ£?¢Ñœãý}(?ïb̫ѝ«?¢Ñœãý}'?I š&tŠ¹?l)ËÊ9.¡?ïù·ÙvbÝ?l)ËÊ9.¢?Ég·"}?±¦9Á×Þa?ë¦>!?±¦9Á×Þa?vÁ§§+?kÛmÜñå?ïÓ|°°å?kÛmÜñå3FGL J1740.5-2642?ôÞ i—sO@û¿¼CÎÀ8ÏËRyI˜À:µ½Ñb^?øºQO}ì•@ìG'd?ô4đ?¿±ïGºU†,¿àìi9i¿æIæ¯æ¦×¿ïe­¾ê‹úUNASNonenone?+J½C™¢Ñ?(lZ7.*?ïþKT+Æf?(lZ7.*?Bvó¸²?Tãâh´Y-?ïûb{Ã?R?Tãâh´Y-?oû{«ç?…ò Ý~?ïŠ@SÑ?…ò Ý?¢ô•ƒ?sŽêRA=?ï¹ùt-©ô?sŽêRA=3FGL J1742.6-3321@v>p†nD¿üdóºw_³À8)+hc–¨À:wfÀ(yœ@kä'fI‹@˜?&†}?öñ ԋÝï?ËÄÇ>\Jó¿á†ÿI\ül¿êôϺÜ¿íô[L
lUNASNonenone?(º,¢7¦N?&¶à%ã4?ïþt]5܅?&¶à%ã4?0ß±îç¬?G$³|³^ˆ?ïýü$	Â#?G$³|³^ˆ?tð3W÷a½?gpϔ©-Ä?ïÖ™P=?gpϔ©-×?gŽû¢íC}?Z'4æÑZÃ?ïèq]¼?Z'4æÑZÃ3FGL J1744.1-7619@sѬ<žìÀÀ6x›ÇqC9À8"{?;2À;]"mé§@W±\®×™@'p\"y?ó¼†=Ç5ß?të¸cËäÀ¿Ù&t;™½¿åÉâܦ'¿ïÿíkÜOªUNASNonenone?‹Ém9Ls?•´‹—ŽÎ¤?ÚKÏ?•´‹—ŽÎ¤?kG¯¨ê?tè‰K?ïär¸PW?tè‰K?§¢šÎ‡? w«ÊUú?î…ÖS׏? w«ÊUú?Ueç¹¥éê?K.þfr§_?ïõM#-
?K.þfr§_3FGL J1744.7-2252@N8C=lr@
©‹XߕÀ8¢Á¾{Ñ2À:Ò('fvW?ý 'b"s@^ߥ—~·@÷§üÞ¸]?¸Ø>Óp¿ìZV1ò¿çRg!]ƒû¿ïÿ'Õ/FêUNASNonenone?ºMŒ™ŠŒ®?¿<ÇHòŒ¤?ì¶Nlήj?¿<ÇHòŒ¤?€«
­&;?˜MAm;>Á?ï¹ýSÉKg?˜MAm;>Á?ϹñT'Ó?¶ n¼>#ß?胪ß|Ë?¶ n¼>#ß?'ï[2ö?€n]µäρ?ïoˆ…'fh?€n]µäρ3FGL J1745.3-2903c@v}Ò½<6¿"" 
êÀ60•âTôÀ8¥ãÛÝ@%{‡ŠÎP@	ùù€´ñ?ô¡9óÁ®?æÚcY\ë¿à'î}î垿ç–Ûñz¿ìk]ãyÑAUNASNonenonep?,š·1™˜B?'<ÞÝ3Í?ïþ6TŒæf?'<ÞÝ3Î?'4sØõoH?D÷©*ü?ïþŒ¸Âpª?D÷©*û?rœW´Öa¢?WÖ	á­}?ïÚÇP–S<?WÖ	á­{?:RžIk ?:%Ì[3c?ïüµ¿6Ó?:%Ì[3d3FGL J1747.0-2828?áÔG '¨;¿¥(ÚûÊÍTÀ6¦¤Gr…YÀ9Æé]ý@úÁC`Ó@ÂÁ†º?ûtS5G¿Ä34	òÈ	¿äÅHEWç·¿è]xãQÛ¿î"ËÝUNASNonenoneP?ÀÝÆü?Ơظï+f?ëÿ|HŽ@ý?Ơظï+f?KwÐgtØ?eR%¶í!ð?ïù"æ"Ê?eR%¶í!ð?ÑÍ "±î?Á,(úWŠí?ç/¶v'
?Á,(úWŠì?€êóD7þ‹?|\Dêñ£	?ï¼T2ï ?|\Dêñ£
3FGL J1748.3-2815c?ìà³3ž"¿Å#rö"À7âÃ2ðUÀ:h)qéQh?ÿ'´µÔ¸©@9›
²ái¿þÞ²G»U?åiáypô?ƒ4K´ýÙп͝D¬q&¿ê"ªúƒÙUNASNonenone$?Æ÷Ûç³85?ÕÀÝqôN0?êB	1ô?ÕÀÝqôN0?'û³-'Ò?¸…ÍäÇÐ?ïo "f"r?¸…ÍäÇÐ?Ë~éºc??²z´âuÛ?é8 E'g0?²z´âuÛ?€àÑýêêB?Œð쀾ùV?ï¼|¸TW?Œð쀾ùU3FGL J1749.2-2911?ȦÃ"Ôì+¿êתv`¯À7Í«û›í1À9®"ñ¹ì?þÐâ»Ìtb@
ۼܿ´?õ$ýÍð
?ïíßvȉF¿Üن±+þÙ¿çLÞ±ëcÖ¿êÅùé‡åßUNASNonenoneD?O9	[Ø?QYÙ՟K?ïø1½©=??QYÙ՟K?E" ¥ƒÍ*?^À>5¼êt?ïúš÷֟?^À>5¼êt?… ìAàjã?‡_b]ì?ï©|Nø~T?‡_b]ì?ˆIÀ
çê?õAFىN?ïžØÿÔc°?õAFىN3FGL J1749.6-3133@vcpâÁ*ØÀ×)9µ-tÀ8²²eByøÀ:u'OÐ!ì?úHDºšH@
ÒòÖ¡¸?û|½›+•¿ßäk•ádp¿æîrÇÑC¿æŸPµ¥ô¿ïÿƓðÖUNASNonenone?Þ¿—I5;?Òw""Žð¢?àú 4[eb?Òw""Žð¢?©Ð&o¼?¹TÇC¶Ã?îgâý™ô?¹TÇC¶Ã?×ÊUÚ|m?¸ Ã`´£?äÕÁýJ?¸ Ã`´£›?ÆeçS`Õ`?µ²'Í_?êf†+'ʨ?µ²'Í_3FGL J1753.6-4447@u±]ÌcñAÀ"Õ5†Ê‰üÀ9dßý+9jÀ;cìƒKy?öPrß­*@
·²ˆÓÏ?÷Y˜1å€M¿Ùl°f:¿Û¹Š¹	ª¿äT*\¨€¿î·(ðmUNASNonenone?BÚðfO?ESp•1J?ïûICýúf?ESp•1J?rfÉáPV?'zxÔ°?ïÛ2lx½_?'zxÔ°?"p'ÖFâ›?…©ÄëÍÔü?ï\{qMÈì?…©ÄëÍÔÿ?¦ïja†®Õ?iÀ4Û
<?î'	Yç•?iÀ4Û
<3FGL J1754.0-2930?ÜÖ¦ YŸ¿ýÊÌ&´Ÿ¯À7çå7&ݺÀ:2ËÏvË8?þ_¿c×ñ@[çÿ@G$êp Ï¿áÎ*2-¤©¿æ¸€"åÕ²¿ëÁþ¸,VË¿ïü»8¿}ôUNASNonenone?†¢)7Ms?'/:¦é'¡?ï¥w[ï"Ë?'/:¦é'¡?K됡Ö?b–£RÝ?ïù8Å׊?b–£RÝ?Ąðh–¸?²m­­Ãsu?êÞÃåÚQß?²m­­Ãst?Œ({
X%´?à«ñFm?ï^֟i?à«ñFm3FGL J1754.0-2538@?§ëkôE?µ»Ä¼²ù<À7æyó$÷À:T9ܚ *@wp×ÙpI@ÏôTüÊ?æގ¿‡%4?ïÿ¸$B`¿ÑRôþˆöM¿âaåí"¿ë#‹²(›UNASNonenone?Ö68FKQ®?Ô´(`¥m?ääãÜÚW)?Ô´(`¥m?YâSëî?'úX@Ét?ïóÖ@
}?'úX@Ét?¶''n‹\?®b²6Ûn?í-½-Ò."?®b²6Ûo?•ð":ê!?Œ£s¥Ÿ±?ïP{_Î(¯?Œ£s¥Ÿ±3FGL J1757.7-6030@tÐ,<žìÀÀ1*$š<À:W"'iÑUÀ<;¶N?÷6&:&l{@{QZÀè¿óñF×Tæ?jiЬ<øÇ?ßÏ|k¾¿Ï	K®)I¿ë¹KÕZSÍUNASNonenone?ΦaèiÍ?Ø_Xšõ}Ì?èVg¼ÅåŒ?Ø_Xšõ}Ì?ÀK °Z?ÑXêþœnz?ëí?·Óøé?ÑXêþœnz?Ñ²Þ ¥?µuŸI?ç&ïý÷-?µuŸI?΅9ôBð?É)ì?'?è^±'ïCú?É)ì?(3FGL J1800.8-2402@ÓW>«6z¿ÜíWœI!\À7VIÿ''ìÀ9¶0©ë÷?ûepÈ@½ÉljÁà?ù1%'¿Ò
'ús¿ãÈÓÉ@PR¿á_)oÁë¿èᏄ—ÔÈUNASNonenone?t½Y4·1 ?w>q ë6Ô?ïօM–'ž?w>q ë6Ó?aÀ5q`Ö?vl'D3?ïî<ʎ ?vl'D3?Æj~0"çm?±åÖp¢ÃŒ?êe`sÛ%?±åÖp¢ÃŒ?¥¼/åbš?››aãI$?î¤=©ßÆ?››aãI$3FGL J1808.3-3357@v`÷<ÉÀÚ\¢˜EÝÀ9w;ØbçÀ;DŸqIï7?ø
.j€@oÅz¤6?ôž9ŒÈZ¿Ö¾l$žù^¿Û‹ÿÅ*¿çVïó9ëV¿î°¸ë!)NUNASNonenone?PT?–F‰?P'à¾?Gž?ï÷Õà4Ý?P'à¾?G?‰"Szч%?œ]Ù‡î?²¹ã?œ]Ù‡ï?¥/Rìþ?šáµÚL?î­ªÞá0?šáµÚL?´¢šÃ¢q?¢n÷{39?ík¬§‹±Ý?¢n÷{393FGL J1813.6-1148@2OµIùH@³Œ|z¤âÀ7ÁÐ\¤EÅÀ:¾­OY?ÿ"VÔxß@¤[©ôۊ@¸½ÄMc¿ÝˆZá'Ĩ¿í7úb˜b¿å
V<-E¿ïÿYƒ÷=[UNASNonenone	?–{p˜9'ð?¤õ‹§H~"?ïL${>3q?¤õ‹§H~"?lèz«a 9?—j\C¼?ïã…Tžß?—j\C¼?̉6É7Ç?´µë©/?èý²M²?´µë©/?bt!súÛ?`%W¨Ê·I?ïí‹ÞŒù?`%W¨Ê·I3FGL J1823.2-1339@1š¥ç…µ·¿¸€,5=$À7jf¦'GÀ9R[Æ?ùJšèùÿ
@䓳%±À?ýwã:"¿Ø`ð"¶—¿à¿Ÿ×eü¿ä5†‡8¿è"†¸ýsDUNASNonenone?p	¿½#"¥?y$8ëò	?ïß쀅¸Ù?y$8ëò?_ñ§Lî´?q{ä'±?ïð,Yý‰?q{ä'±?Æ5AaSÔä?±ØO͒l?êr¯§«
Ç?±ØO͒l?¢ä±äíR:?–'.GÎõ?îÑ´á±*Ü?–'.GÎõ3FGL J1827.3-1446@1ud0+A¿÷½¢!þW‰À8ˆÿI ÛÀ:•ýʛš%?ö'Ò€@
'Ü®—,­¿ía'ÞÒo	?çtÝ̃¿Ï(œA8ž¿ßH–3€¿í³rB_ŠUNASNonenone?ÄÑËç+L?Ô6ý™??êú‹5-?Ô6ý™??–ìÆ×Vg?¹ËnU`–?ïH™ÉELÉ?¹ËnU`–?²«p™*ÿ?ªhåDD~?íª'ìÚ ?ªhåDD~?§³ñv#?¬¶í¡Æy?î"À~?¬¶í¡Æy3FGL J1831.6-6503@tŸ?¼À6gø"»ì«À:‹†³
&À<e»À5Ö?øð+oð@"˜ýgtX¿õÇlãË¿å뒙0yV?Á•î¿:èß¿à8ƒÝ£<¿í…̘IhUNASNonenone?äҁÜ|o?Ù£¡W¡ë?×àZüG$?Ù£¡W¡ë?¯Ôh¯2®?Ç©ÁPš#Ú?î·)uÕ?Ç©ÁPš#Ú?Ԅ³öʶ?·Ê"ÙØôå?彦÷¥?·Ê"ÙØôä?¡JÑø`Ûï?­ûeH.ñä?îëRàyòB?­ûeH.ñä3FGL J1831.7-0230@<u^á6ç@	Ó˜K$ÂÀ7àùx&'KÀ9ÆõkQ‡²?öÉLÌKž@»PÒ@´þh{>¿ç"=ý;ª{¿èóAç½$¿êF$mƒÍ;¿èõM¤E£UNASNonenone?i1ö¸<Ç?{•»®l'?ïæÎ	GÃ8?{•»®l'?±9Ó¦¼D'?æÇÌï-?íØŋ(wo?æÇÌï-?Åßµ¾rµ?°툾òÀ?êˆ=ҐcS?°툾òÀ?…¿âC²?jCýމç?ï©wÂóÂ?jCýމç3FGL J1839.3-0552@:S¹EÅ¿‰ÕÓ0¿ À7±EˆÀ9SÓ[\G)@cªpCµ@ûÊ"x{?ù"ü(¯÷¿´Æì`@&¿Û̕asû¿ä徸âà
¿êës§¨·*UNASNonenone?0ÙÂFV?-BÛ=º>?ïýäÇ¿˜?-BÛ=º>?.N–îjo?Gñ`V·?ïþ'^?Gñ`V·?vš¨—C°?lå-óg¥x?ïÒʯüÑy?lå-óg¥o?^•Žõ‹ž?W™3AXÂö?ïðµ8…:1?W™3AXÂö3FGL J1843.0-0359c@<mCx$Õ?¦µ¯`À86(ï'µÀ9Éh%ƒGH?÷Çy8¦È@š#WH?õÑÄ ÙSï?ÛÁòu¿Ý˜˜ÊLü¿äh˜pàÎó¿ïÿÕÄčUNASNonenone1?˜íÞìíâ1?¯yUö?ï8'˜ï?¯yU÷?{OÝ^êbÓ?"pâ}Ný'?ïÉ`EB+9?"pâ}Ný?¨°lSy?žÓ_EʹX?îtù>oÉ?žÓ_EʹW?¶_…°Êà?¬ž%é"š…?í4Iæ£ü?¬ž%é"š"3FGL J1843.7-0322@=çáüú?ƍ¥šƒÏXÀ7ªñÀ9À¨á59ž@"Ùz/F@'Ý<Ü@CÕÖᣟ¿Ü;š<#>¿çòµ0Æ=ß¿êmIçՑ¿ïÿAHl"UNASNonenone?³š­®}9þ?¹<_D¡ø?팪J0XÁ?¹<_D¡ø?>'¡0XX?S‹ˆà<…?ïü;Ùõ?S‹ˆà<"?Í5Y{i?³"¦Ð+ª2?è²¾)¡%¼?³"¦Ð+ª1?zŸ=¿ë$?p'*
üa‡?ïÊÁ"€)¶?p'*
üa†3FGL J1844.3-0344@<˹M"¿ÂŒæÃCBÀ8I­Ï±ƒ›À:9ºHf?ûîÍÕý£@j#²Œ¯¦¿Û´ÆVø?ï÷sB܍N?Èé"}m¿á_ûÎBÓ¿ìtĚúÝUNASNonenone?µšNÂgV?Ìõs0¿3?í_,¶'³?Ìõs0¿3?ƒ_'æÉxž?¬ËEDH?ﲃ`dÚ?¬ËEDH?¨–û½¡L?©jƒ¨òí?îv– D%ì?©jƒ¨òì?"¬s4Ø{?•eljž#?ïZœf['<?•eljž$3FGL J1848.4-0141@?…fîW¿¼Öpd—gÀ6ã¸WÊÂ1À9‹‡Öùvy@¥cSa|@´Üú‰?ÿSqç£è¨¿ÔàÜJ»‡¿çÈPó¿æv×·%_z¿î"Í]UNASNonenone?bÀ-«9øI?t=¼Xn®?ïí?ÒTÆ?t=¼Xn®?3ûòT·m?Lë–—ìn?ïý€µi?Lë–—ìn?¼écnRY?­å¹¿Ïh?ìbӒ5½õ?­å¹¿Ïi?f~ËAÓ?b‰[Té6?ïéÿí4¾?b‰[Té73FGL J1848.6+3232@O$¡œZ@-| fèlÀ8ãÌґÀ:]vfœí?üÑÂèbÒ@{þÔü?þçÛv]ÕH¿¤\¸råµ-¿éôsH»Ê¿å¸±Òø¿ïŸaæ`,øUNASNonenoneP?îüMAtm?«gx!'֔?§à;+è¹3?«gx!'֔?Ç(Ú?ž`YìKŒ?‰•N5É+?ž`YìKŽ?çܧ¹Â"É?²¶7ž¶H?ÐF°ŒzØn?²¶7ž¶H?ëÕÚÍ°¦Ê?¸º"'%Œ(?À¨"É=dÛ?¸º"'%Œ'3FGL J1851.2+0423@Bh"pdìê@d}€^_1À8'­K'E¿À:T\Rn?øè뗾"@1+¼ÇF@šO'ã—¿¿ãŨM!Ø¿ëÄ7Da¿éF	Ï*N¿ïÿÚLÅ´UNASNonenone?ª`sÅDú?³×s±ÁÔ?îYøÎÓ«°?³×s±ÁÔ? >÷áp¦?·^~uú¾ô?îüŽèö?·^~uú¾ô?ÏÏʄ<˜¶?·ù»¦£W®?è
^ðÙÒ?·ù»¦£W®?¡»³S3*\?•ŽÄ$Vû?îäDÊÌÍZ?•ŽÄ$Vû3FGL J1857.2+0059@A<YÈÉ2¿êçLàƒböÀ7À!)Es¨À9wúÊ6˜?úSÀý
Ø @.…fîW?õRtK×Cô¿àû[4û¿ß£†ŸcT†¿áNnokÀ¿éE1çwcUNASNonenone?‹ôøÒãíº?"H¸B÷k¨?ï,´pJ?"H¸B÷k¨?¨zav/?½¶ýÔÕì7?îxYçèžî?½¶ýÔÕì7?¾,Æu¹^?±Ì¸éƒÌæ?ëPtÎb'¨?±Ì¸éƒÌç?¿˜˜VåÜÌ?µ+mÚ?ììõ#Df?µ+mÚ3FGL J1857.9+0355@B•Î|Ð57?Õñ÷(ÀéjÀ87¸Óñ"À9Ü7i"ÙI?ûMFˆï@Cˆ?ÿõ?úÆ3
nmò?ïšÞw3#¿á•¿Ù8/¿êºÜÓç.‰¿è"HÒõ UNASNonenone?xSYb\dà?…z â[éS?ïÏYM;G6?…z â[éS?–ñ7#³Z?²tÚZA¾?ïHvG¾âe?²tÚZA¾?Á0[Tqñ?°|Ԟ¨?ë³é*ã?°|Ԟ¨?²¦Ÿë[j\?¨ÛKp"?í«,"'´?¨ÛKp"3FGL J1857.9+0210@AÍÄupÅ¿ÝyO܌À7iKB±ÂÀ9³ŸAyG?ý­åSViC@dõOÍÈ ?þ=Ž@u"¿äf©#Ǩ¿ã3"]¼¸q¿æ÷ègï
Ñ¿ìÕZ›¾CUNASNonenone?4³ÅĨü?/¬Èxã­á?ïýi‡]Çl?/¬Èxã­á?CnÛêNÆ?ZsoéÌՓ?ïû$z‰m?ZsoéÌՓ?Jà០?ŠŽjOø?ï}¨øó?ŠŽjOú?"¹)Ž­ÿÑ?y"‡èª¥?ï­YÅH?y"‡èª¥3FGL J1859.6+0102@AeUÅ.rÚ¿õ¶âdä†'À8
šôãlLÀ9ј:ôÉ?÷i§¡D2à@éüíÑÕ?ÿ'%Ÿ í? I^Ó&¿ãoòÿïíl¿æJÀŒ¼UJ¿îŸØ"UNASNonenone?qúwAÍfæ?ÕÄæÓç
?ïÜ|e3?ÕÄæÓç
?°IP%p?¼H|æ/?íÿÕûQÿ?¼H|æ/?²®,"»?©#È£?í½J:mž)?©#È£'?Ç+r6ì…?¶¢©=̺	?ê9õ#rDß?¶¢©=̺	3FGL J1900.8+0337@BœæB¿˜1¿Û£Òm¾À7°]«¬Á•À9ñïÞIÍ?þ9ì$ÖÏ@›,ªØÜ%@͵^q$…¿ÓfÙJVê¿êt–Ë'–ô¿èèæç]п/âØõUNASNonenone	?_ó®/{…?b•Õ€·bÔ?ïðr(èC?b•Õ€·bÔ?F÷.bÇ?a¼>íun?ïúB=4}(?a¼>íun?ÅöáÞî'ô?³›Gg"¯?ê'GˆD[D?³›Gg"¯?^/'Ûå
?x÷œ>úô?ﺇAôl?x÷œ>úô3FGL J1901.1+0728@DXÁTɅð?óþäǕUgÀ8.üóEºÀ:8*ù?ù霾è¼@
Óô²š@}…¬o	¿äen¿æ›Ž^RÕ¿çnÿ¿Ø¿évPŽã³UNASNonenone
?‡|ä—´P?5ºi~?ï¢o¡/?5ºi~?¥8.Ûl	Á?½KìOš +?î¬}I?d?½KìOš +?Ã{°Ø?±F¬>ªòÂ?ë!"Éú?±F¬>ªòÁ?±¡ÇMp?¢™ÙƒpÓ?íÜ+ÎGR?¢™ÙƒpÓ3FGL J1906.6+0720@D˜±_ˆü"¿œ6‡P–ÆVÀ7îü¢}nÀ9áa£‰¤@'a–óÍ@
ØK)tª?ü¢üSøû¿ØŸtùÀå}¿âhÃQ46O¿ãî¯=B¿ê"G§"]UNASNonenone?IÎÃõé\?PZYfY¯þ?ïùŒ|O†?PZYfY¯þ?)Žì˜lV?Dۓ¢zȏ?ïþc¤!6y?Dۓ¢zȐ?Œ4¶qä‡Ó?‹CâǼ?ï-&8má?‹CâǼ ?WÇ\¹Ÿ%?Oh'©¶z?ïôQ£0n?Oh'©¶z3FGL J1915.2+0954@F9q!«K¿æ'"€zä£À824Òo£ýÀ:3î*ëf?úL0':+ @TYsŽÃ@Ú1'w¿ÕZ8äD…¿êÀ>/ÕI¿çÙŒ/n¿åó¡:!ä×UNASNonenone	?•¿7@<÷!?§²´Ê2b?ïREþH?§²´Ê2a?±xdG²C?ºßÛd€?íÐîSw	¸?ºßÛd€?Ó	Êdço?º',`f?æ{ÍÿŒI?º',`f?½D$üRS8?°.
«ê?ìW{`uµš?°.
«ê3FGL J1919.9+1407@HZåÿ£¹®?Îó_ތè±À7Ȓ¡WÓüÀ9õ¦gÞ5«?ö{ëV¦@ܲ_Ž0@|®fÛ+_¿Ýº}ºjõl¿èR	c¥¨¿èqþÂé<¿æNkwQUNASNonenone?¸ ®iÉ?»
vÔ\nš?ìýküª2Ç?»
vÔ\nš?ÅјQ?džeàÐ?ꋙë"×?džeàÐ?Ö+äŽý‡?»?f$1¨ì?äê
¸ñ=?»?f$1¨ì?ÑAç$àÙô?»z^³¸?ç_m"?»z^³¸3FGL J1921.2+1506@HÝø>Ÿ?Ûi' hÀ86uT?ó5À:V‹"ÞQ?ÿ̒_"Žh@ƒjY5@´s0T¿Ä7·sÁ%¿ë§äO‡¿î•Uël¿îfžšŠZaUNASNonenone?ªX"çN?Ãñ-ÐÅ?îZ~—±Ž‹?Ãñ-ÐÅ?@7;K?`…o-Á–v?ïûüûò1-?`…o-Á–u?Ècãj©ç;?´÷
RøQì?éç%U†1?´÷
RøQì?rŸCÃ@Ìw?héþE#ð?ïÚÁxy~f?héþE#ï3FGL J1925.4+1727@J%]Äuq?äp?ÎL(ÍÀ8•+á/ZÀ:`Þ	53?ýj0'|G@Ûtä®jâ?ð¡ç¹b6׿Õ9n€ç-¿Õêߑt|¿ëÉ7»qõU¿ïÿâ–b­tUNASNonenone?r¯ü>2–??•dž?ïÚ ƒšÓ?•d?7¶™'³Š?Qkì½Æ?ïý	,Íɏ?Qkì½Æ? B…'Ø•?šŽž@×?îûצâv¯?šŽž@×?ySHuLf×?q z©Öœ9?ïÍYog2?q z©Öœ93FGL J1928.9+1739@Jm[[Õ?}&3ò"'À8imOŽ³À:4››ÒXþ?ú@ÈÍcˁ@òlÃ!Ó9?úgRژgj¿á1ç)€"¿åQƒ8aÎÛ¿åÇ[sÄ¿íµ²ÔÔUNASNonenone??Z9=DåÓ?@Ŝ|Ž¸?ïü¸ØWc?@Ŝ|Ž¸?b]Ù¥êP°?u¹kÀ²D+?ïí¢&Z¯?u¹kÀ²D+?±'Ž´Å?¥0ÞýðÉ?íÜ»)g`?¥0ÞýðÉ?¡‹Í5aì?•G圆?îçOC,©á?•G圆3FGL J1946.4-5403@u~6z—À=ûH
[À94ìð{(À;µû-2h2?þρËDz@
r©rՊŒ?ø·÷'¿7?×¼ê×yÏ¿à܍¸'¿è½ãJ' V¿ìýco³c'UNASNonenone?FñÐ]E—Q?FÙ{k³Í?ïúC‹è®š?FÙ{k³Í?vÒü4ˆËó?€EÁiÉõÜ?ïÒZ–îh?€EÁiÉõÜ?Œ'´í©"ú?"D(æ¹·?ïa,IYí?"D(æ¹·?n$Âêdw?`õßÇQž¾?ïáÛ=›õ?`õßÇQž¾3FGL J1949.3+2433@NšiƒQY¿çCM\ª%À8ÍSù|X@À:¬°',ãŽ?ùƾ•|@
ï/"Ã?øâÞ0¿Åçö-z¿çnKŒ	Qý¿èJ6F°_ü¿ïýÌø$ÙUNASNonenone
?v}_ý	¡ç?"aUXWê?ïÓ@ì¼?"aUXWê??Ùéwƽ?W&­7¸?ïüÂÑ)?W&­7¸?ÁŽÛý?°6®ÅÕo?뻿yI?°6®ÅÕo?Ž¦Âߜ8?~Õg)‹'?ï‡ídô?~Õg)‹'3FGL J2017.9+3627@R¢ª:э&?ÚIECVÀ7tUóQ›ÔÀ:1GNs*š@A(¯ ¿h@
{œüOœJ?ö"|ôÈ>s?áô3ˆî{ž¿ßå: &)ú¿è§°[…•^¿ïh]QóEeUNASNonenone?Êèü܃?ß;ÙÐ.j?ïÿ	¨¸ù?ß;ÙÐ.j?$
ç²×¢?BVª±gM?ïþ¿/Á"Ó?BVª±gL?r‡ö¢¥Å?TÚ\ë±×ì?ïÚð亵?TÚ\ë±×Ø?/<jýÜœ?(¹·Þ´k?ïþ9P'?(¹·Þ´k3FGL J2023.5+4126@SÐ:>À/0@»|,ÑðÀ8"Ð=1À:pñÒ?ÓU@hòbˆ‹@ ŠÒ+†l@BMec‡¿Ü:&ôØÑà¿æW?ÁQ!¿î^måû`οأ>ÍUNASNonenone
?Óã¼D}?Õ-]_ª½?æ!ÝÁxö?Õ-]_ª½?½Ñ|•\?Íj–öÓë?ìEÐm_ô}?Íj–öÓë?Ú'ùÝ8'?¸»Ù=D?âìvc¾?¸»Ù=D?ˆP
UÄež?‹·_3QØi?ʨîi?‹·_3QØj3FGL J2024.6+3747@Säy'¼?°«'¡Æ3À8¢×áÓÅÀ:vXò	8?ú*W‡PkÓ@MjàɃí?ý©£A«q?ƒÆó¿ë ǾΏù¿á8ÌÈ5‹¿êú¿»ä"ŒUNASNonenone?­.R8ôu¨?²ƒˆƒÙLO?î-Üp¸¥?²ƒˆƒÙLO?"˜;Oýé?§/rÚú?ïc>'…€?§/rÚú?Ì6_ Fïã?³Û%Áe'Þ?èòh7îD?³Û%Áe'ß?¾ÍµÅ‡zf?«Ïk€Óî?ì&IGO´?«Ïk€Óî3FGL J2026.8+4003@SŸ}€^_1?ðf¬ƒ§ÀÀ85>˜ÂEÀ:S½ei?ýöâõÙ@ð}0Ò?þ̌ÐÞT_?î´®>R‡H¿ê³¯J¤Ð¿èÏÀG¶Öt¿æQA~6UNASNonenone?È;é+b:¶?ÈE%«t?éñµ'qR?ÈE%«t?™öüÙÒ?·ÙZ29WQ?ï3€H1p?·ÙZ29WP?×èˆjÈå?ºÐš©.?äz»Ê›?ºÐš©.?¤‹¢žãÿ?™»Ua…»‡?î·EÖÎð?™»Ua…»‡3FGL J2026.8+2813@Q5éÍ³}ÀK5°»õÀ9˜d
ƒ À;:†œfÓt?õà—Ê·sÊ@ᓿºëy?ùj§ŽN⼿â2kü¿Òs=idj¿ï†)ñk¿ïýGwtUNASNonenone?§¹'úÛ?¹‰—A--?fïR?¹‰—A--?oRvwo?"ò/£¥• ?ïà­ë‰ˆî?"ò/£¥• ?Àÿc̟f?ª)Áæ£hX?ëÀ'Ø&\?ª)Áæ£hY?'­C¸óZ5?…w°Â¶–í?ïr•â8e.?…w°Â¶–í3FGL J2032.5+4032@SàÞ~¥øM?Ü
#$G]À7 dJ,süÀ:*†ƒ<`@÷øµ"@;U«3@˜­×êN¿Û‰å—=¿èÒ~?ԉã¿ïÿÌÔY‰?ïÜn~Éð¶UNASNonenone?ìv">pys?É
(ÃîMà?¼Nî|4m?É
(ÃîMà?æ!X¡0Ñæ?Õ(nBeWŒ?Ó½N½ž\3?Õ(nBeW?ä<®¸_"?¸t_íêm?׆¢A»Ò?¸t_íêm?ëÊFÏÌ?È7y‡B?À×ã†äÀÑ?È7y‡B3FGL J2032.5+3921@S¤´·,Q˜¿Ñ0l娶À8,Áúá³À:T
ހS?þ/}Ç/%@3'W°ëñ?ûÛ@bƞµ?ՇW€M÷¿ä¥fÁÕøÅ¿ê`*èêmO¿çºº•VƒUNASNonenone? FGgßò?¬jy>š–?îû›Ž)'?¬jy>š–?W´ËvŸ¶?tâËç\Ã?ïô%špD°?tâËç\Â?Ëø/½iç?·söê*H?éô›å‡?·söê*I?‹}§N;3I?€›AÀ¼ì?ï'	bÇ3?€›AÀ¼ì3FGL J2034.4+3833c@SŠOv_Ù¿ð®â5ꝘÀ8^ìÔªÀ:‰Ë—B§D?ú&ñ–…½ð@›àÆ©È@;¢F¨0¿×¯‰Uw¿ë
¬ÑÚ¨®¿ë †?A*忁
cgÞ>UNASNonenone4?ÈÐJð?ÅQä¸?éËí|üÃà?ÅQä¸?ؓ&¢Çl©?ÓÔó)ý?ã¶l®œI¬?ÓÔó)ý?Þñ`ü«lB?·=Ò=™Ã?à‡OªIß?·=Ò=™Ã?Ù!«6·U?ÌÅ(á5Â?ão*d¤Us?ÌÅ(á5Â3FGL J2034.6+4302@Tq?l&š?ù¨·^¦~"À88;·f3À:bþ;â?ÿaºÅc@
ÉY;°…C?ÿ¾–EÒB¿ãRêCçG¿ã¤Š÷t¿ëpK&L£¿èáX'€_PUNASNonenone?vͽÃEwX?{€Ï'î?ïÒd"yu?{€Ï'î?rãÎí8ã?¦X3q§Ž‹?ïÚ8b%à?¦X3q§Ž‹?ÈqçÄ˨m?²³÷£ª$4?éã†Íå?²³÷£ª$4?{•Üôìx/?r‹;Ù«} ?ïÈÔF'?r‹;Ù«} 3FGL J2035.0+3634@S(ˆ&ªŽ´À†»øiÀ9°à<4À;
-åìY?ü«äåS@²ìì§Þ?ÑNÓã:?ïêÖò"[3?™é¢à.Y¿Ö¡CU®÷é¿ï0#ëËUNASNonenone?'¦	zÀ?¶þ6Ç$j½?ïwºÏ´)ÿ?¶þ6Ç$j½?ŠÐZØ|šm?°m(¬V?"ž
–?°m(¬V?À—¢Uõ"®?¬ìd%pµ?ëÚj'›?¬ìd%pµ?°ïì>àùç?¦Ô@83©?íâx#àÃ?¦Ô@83ª3FGL J2038.4+4212@TaÄØì–?á]iR‹¾À7ö;¤ñ¼pÀ:ûwÛð?ÿSÊ7F=Q@'<§P;'?ýC7àlõ¿¶ÕA™(¿åæà/'N¿ç°—já¿é8‹ÛÀÛUNASNonenone?TÜBwi+X?R­o;Ò/¤?ïõ'ÞÄKj?R­o;Ò/¤?\ "	˜|F?x‰™kñš?ïñï½û3Â?x‰™kñš?·®"¾Påo?ª;Q"k°t?í
;¨5ãR?ª;Q"k°t?þªHF–?"¸hùÁí±?ï€VÞçÝ?"¸hùÁí±3FGL J2039.4+4111@T5¨mqó¿Ê'¼£nÀ8û'²õ‹À:AàLÜQ¥?þìñÓA†@…̘Ih@ê:Ì.Â5¿×´È\ƒAF¿èPÎáÇR1¿ë58~v¨~¿äÝaeÎUNASNonenone?'ÇӖRÑo?ž/Dý¿&Ë?ï´à±¦´º?ž/Dý¿&Ë?{IïQÔé?¡hP¿¸ó\?ïÉl!\V-?¡hP¿¸ó\?ˤm')óÐ?»ûöÃÿ\R?éä¶5ƒ?»ûöÃÿ\R?Ÿ3€]?‡l·o(?ï{c"ý?‡l·o(3FGL J2039.6-5618@uS²þÅm]ÀB"Ùý6÷äÀ8ʇkŸ‹À;O3·½q?úfý4Ñ@Y…kE-?û-x¦¯×Ÿ¿ÑӂMø†d¿ÝÝ'ãɾz¿ãˆã˜/% ¿í×)5óUNASNonenone?Y[Wøö‹Ú?V~0z=5?ïóRT"º?V~0z=5?"¤n
ò1?œÐ"'¥Ù?ï­nGÈ7·?œÐ"'¥Ú?Œ§}3HàÆ?‡½#—í?ïb2Ü}?‡½#—ð?~#² …­?j‹œŠBW<?ïø›ü¾ô?j‹œŠBW:3FGL J2041.1+4736@U…Ó™o¨/@±€%TM_À8+Yª–AÀ:ÇvË8x?ûöžšŠZa@…4"@ÔŸgd¿×bYäfü¿äÒø/§Ÿ¿éN9¥Ni׿ê(±Žû'vUNASNonenone?‰¦¤óYß?ŒN ®™\?ï›áel2™?ŒN ®™\?ˆ(ó+ètÁ?£~m¡kû,?ïŸ\3P^-?£~m¡kû,?´Nq ME±?ª^u³äÚ?ív1ËöWJ?ª^u³äÛ?"
"eÊ(?~Fr#´\?ï_"ÜÓ®?~Fr#´\3FGL J2042.4+4209@T{ªOÊB¯¿²;X6LîÀ86‹ò)ôÀ:UÊ! áø?ú)Œì7 S@GØ4ß۝?þíâ¦Ó¾Ù¿Û¦IŽ‹Á¿èq®0Ý÷¿ã¡ÄZ"Ó0¿éãP÷,rUNASNonenone?›?&¡"0Á?¢™
ua?ï&ÊóÞz?¢™
ua?ۈ
€ú†H?'Zg3]"?ï¼Õüç?'Zg3]"?Èiáp{d?³—c>jÒæ?é凣ܡ'?³—c>jÒå?´%"YUFD?¤8)K­Ì?í{MtÕW7?¤8)K­Ì
3FGL J2043.1+4350@TÕßeUÅ?ëﵩ-‹À8"Íui8©À:· ×æÜC?ùƔ·1¯û@wOz;°Z@ªWk÷ ¿Ü7âȕ8?¿í§"€"¿Ø–§XÁYž¿î"i$ösSUNASNonenone?®?Øa:‡?±é	"?ù´?îyìS×?±é	"?ù´?£é^,%©Z?»'Á'»ò?îÁj=¥j?»'Á'»ò?Ñ>WéWÝÝ?´ºäeôR?ç`ÔT?´ºäeôR?¾bª;š¦d?¯4»M9U,?ì3ª¸Œ«3?¯4»M9U,3FGL J2048.8+4436@U%+ÓÃa?át0‰4LjÀ8|@lÚÀ:à&¶ÁÉ@!­ÎYê­@"R£eö)?üîԞþ2u?Ç`MŸ½l¿çôò"䣿첻尿ïÿ" ¿mUNASNonenone?ÂWS‹±¨	?Ä*l½W±?ëj+•þ?Ä*l½W±?1Ñà;@Ó?H}«ÝÂ?ïýÅÃøž˜?H}«ÝÂ?Ímãw¿?¶7uÇHí?複">>?¶7uÇHì?pY*ÍP}?`²©å:íI?ïßMïªe_?`²©å:íI3FGL J2103.7-1113@BíÐ|"µÝÀA6)Çy¦µÀ9Í#¯1±À;¿VŸI?÷9`üÅ
@N¸Ê·H×?ñЉB37?ïÿxùsŸ¿×¨ùD5J¿â7îÕú⤿ì
Bùú­UNASNonenone?³ÍÁMÜ?µJ‡ˆ9b:?í†GÞö]¤?µJ‡ˆ9b:?ÃçpJÀÐ?ÊÜ3Ëm"Z?ë#íÌ?ÊÜ3Ëm"Z?½©7'Ÿ3î?«äíÅñ½	?ìJÙ
¬'?«äíÅñ½	?Éu	æ‹#?²v¨zÅ?颿}†]7?²v¨zÅ3FGL J2112.5-3044@-Ì`RP/ÀE9nÀY!À8¯¨tþ¯žÀ;N%@+i:@ABŽ@•ä¯—‡Ç?ñĐ£PҀ¿ºTqu§æ¨¿ÐSF"ã!M¿áG¡>Ô|¿ïÿù_|è3UNASNonenone?¹¦-qºN-?Ɔö9ü«©?ìË:Qȶ:?Ɔö9ü«©?…½PT7"Û?'R7%5G?ï©
¾¯#u?'R7%5G?±¬ÖsS±‰?¤ª•Ô?~F?íÊe1•‰Ï?¤ª•Ô?~D?}ëÔPy?p닼Âbô?ïÅÚ(WÑ_?p닼Âbô3FGL J2114.0+5239@WWn.±Ä3@ßT•Ð·À9,Òn¥ÐÀ;ÚPp[?öaÅõæ@)0¬›)?ô"rþ¥7?ïþ,0Á®¿çX/ŽZn¿ê\¼:û¡¿Ù­k+$ÏvUNASNonenone?ê1,õhƒ?ÅD¦AlÒ¯?Ç;L)Š]ø?ÅD¦AlÒ¯?ã˜Ô[¦Ž?×i§$ãÏ/?ØÎWHä²ã?×i§$ãÏ/?åïì6(?´Ï7¶?Ô ä&œ¯?´Ï7¶?ÛËÃ6"?ÅA¶éC?âdó|¶?ÅA¶éC3FGL J2117.6+3725@T³ {5+À Œ$=Ìê)À9´ã¡ûhÀ;[«Åìû?÷º¢˜›Â¿@ImÖr=	?ÿÚ.ÌHî¿Å~Þ]ÕŽ¿å))'¿éˆWHÕö†¿ïÿÃ	ÌUNASNonenone?¶8ùñ…?º>–Fo\?í8íàÝ!Ï?º>–Fo\?p•¯"§"¥?à"v?ïÞԠرº?à"v?þŒ8rH?±­_Ì¥ƒ›?ë\ÿqãn?±­_Ì¥ƒœ?¡·ŽfJ¶‰?…ô=ˆÂÅ?î䇛T˜?…ô=ˆÂÅ3FGL J2125.8+5832@X¯iì,äe@Éú©u°À9'][û©YÀ;ˆ*…È?ö9B×@I@MãÂË ?øÉZí6yº?ÒÀÖc=Uæ¿çmõ*ÜD¿ë:¿»Óg¿ê¨»VO9UNASNonenone	?Ø"ÞMì
?ÊXU"Ø
?ãþ¶Ù	ü?ÊXU"Ø
?ÐåŒq!Wü?Òhõ<Ìd?ç9ÇoT?Òhõ<Ìd?×Ty¶§?¶)K'­üï?ä}UÃ$ú,?¶)K'­üï?•lñ¸ÿ—?®ýÕçý¥%?ëZ¤Ã'À?®ýÕçý¥%3FGL J2133.0-6433@t‹Ò½<6ÀD¢VÿÁßÀ:@ËLš†À<	—@G?ùþð`z¿@B°'¿7Ž?à~ð~‹Sä¿á'òWBT¿Ã4Ì}‹¿é@¢¶½…¡¿ìiµþK—PUNASNonenone?~"+Òf?ˆìï%µ§ú?ïÂש[4?ˆìï%µ§ú?¶0!ƒ*%%?ÇûÐîƍ³?í9ûϚ»[?ÇûÐîƍ´?ÅTá]½Ë?°¬<ñKÅW?êªÇ¨?°¬<ñKÅW?­•zät×ø?§8¶ 4Ð?î&¨Q¸²€?§8¶ 4Ð3FGL J2206.5+6451@Z¡ï^Èt@'W«¸€À92FÀ:ü¹kÆøw?üÁ"\Ð@ef»ü@…újꯌ¿Ïøå!µåÞ¿çғâº8º¿êŒœ",r¿ïÿ"Ó¿¸ÆUNASNonenone?ªh	,öÒ?²yÝú|?îYo0'?²yÝú{?Š­äp?°Däýl™b?ï—ó¹½Ho?°Däýl™b?ϽøÀÿü!?´¯ð¡þ2þ?èÏÀø?´¯ð¡þ2þ?tg'û‡?e2æÇK­V?ï×ó1°ý?e2æÇK­W3FGL J2212.5+0703@Q/‹«`kÀCHP½‡µlÀ9nv½ÌÀ;™FéÉ\Ö?öÙù΍—-@4~…l?ûHÙÉà^¿Ö$;"Ì"¿á*øú¹U¿ä7û"i¿ïÿåFúUNASNonenone?Á¼_cé‡?¿]9zÇ@?ëè'ž??¿]9zÇ??Á,"«¹ú?ÄȗE£èê?ë¾tÚՁ?ÄȗE£èé?·)áÈéì?©Çg	
?íÃÆâÂ}?©Çg	?ÅwÅÐÞoR?®?6Z:4;?ꢋÈd+?®?6Z:4;3FGL J2221.6+6507@[¿Ž`€@ÂQã!¢èÀ9gJöžWnÀ;ç½?ùû÷²©‹@M;G(Þ@…xì?Âyð‹1»©¿æb©\h¿ïÝÂ凮¿ïGKI½ÂUNASNonenone?ÐCèßò	?Ð
ªÊÛ{?çސ{†ü?Ð
ªÊÛ{?à íb'ô?Ë_ …Ø3P?ë7ħ[D?Ë_ …Ø3P?ÓñÔJèä?¶1ÓÜu¾?æüڋ?¶1ÓÜu¾?§œžsÅ|'?•ƒ¨ïî¢V?î†6è=?•ƒ¨ïî¢V3FGL J2221.7+6318@ZÁeUÅ.s@›¡±–À9(‡%ùŽÍÀ;&'d@ò?þQH,>¢R@
;ÏWì{?ü2ßã«¿Õ4o)>ÎÙ¿ç¡äÞ³Ìm¿êüÇ`sª"¿ç"îrA™†UNASNonenone?¾È¯f"|'?¾ç`‰7ÓÞ?ì&ê-{?¾ç`‰7Óß?®áyJ/js?‡L䬬?îèk]	Y?‡L䬬?Ü7ΙϿ?¸m%¨>_Ú?áäó³!?¸m%¨>_Ù?‡Kp>>H<?|¨Qûåy'?ï¢Ò?ß?|¨Qûåy'3FGL J2233.1+6542@[UîËûµ@>Û<ÒfÀ8ɸKgÝÀ;ØWDŠt?ú³
-ºù;@¯}W´@uàŽ ¿á"ŸÇ±¿æ±.–kfֿ놥¥Z[Û¿îljˊfUNASNonenone?˜9ªÅ¦oË?š¸B]PÞJ?ï>2©Ò́?š¸B]PÞJ?ž¦Ñô®=V?º¿Ö××t?ï
ÉpZŽ?º¿Ö××t?Ðý6uè^?¶Íi~ÑÉí?çdôÅÑ?¶Íi~ÑÉì?‹'Qvk?u¼jÂçÄ?ï'öº'žT?u¼jÂçÃ3FGL J2237.9+6320@[&E^®â@öj}L[ùÀ9Z¼ËÍÉLÀ;S:ঞ?÷¼©ÑË\@ T´àó@ü«¶Q¶+¿Ë1Š$Z¿¿ìˆÐí*¿äÉiý
¿ì¦
ÆŪLUNASNonenone?¢¯Ãʪ??¤,(ˆW?îÕ#ÃU\?¤,(ˆW?··(—L?Â"ísæ‰?í	ýßí?Â"ísæ‰?Ö¯Ýtº´?¶zð@ÄÐ?ä¨s'E¢¦?¶zð@ÄÑ?®D*S9´?"Ë<Ô2C?î½^šÌd?"Ë<Ô2C3FGL J2310.1-0557@Qlvò¥¤jÀLø(¡ß¹9À:b8š{@éÀ<5[½•ø?úØ1rìí@Pž¯®?«ɔ•)?ï¢Z´ñ'º¿©‰ì	!¿åèg™±`¿ïÿyOw6˜UNASNonenone?Ô%ì/…?֏Dlˆ?åûíq‰è>?֏Dlˆ?Äêç¤í'?Ò^…Ò
H½?êÅFĶ?Ò^…Ò
H½?Äøb†ø6²?µé2mT´?êÁç^AòT?µé2mT´?¼ï½X‹"Q?µ¤à±oÃ?ìbT?µ¤à±oÃ3FGL J2353.3+6639@]M©?)
»@½?é$À9)ölÙG/À;O{ƒ.J?þCaƒ‡4@
J^Èã3?þi™aܔ?ÒéQ؄*¿èñôgN }¿ì€zŸê|Ç¿í›>ŠTWUNASNonenone	?"G4š*O?ŸiIdÃg?ïeÇn[.®?ŸiIdÃh?f¹A•Ös?|—°ÇºWœ?ïéíF¾j)?|—°ÇºWœ?Щ*'kø?µ» ô§ú?ç«rj·J?µ» ô§úŒ?gAIj7E½?["IãšåŠ?ï辶•Èº?["Iãšå‰3FGL J0937.7+5008@dëÿ´€¦@Gbž À:' €©ÌÀ;ömÏç3€À!͋¹‡ @8e>É…@äÀ^g¿â¯îyèÓ¿ç'Ã&l¨¿åîÏÜÕ60¿à¡xhÐAGNfsrqGB6 J0937+5008?ïÑ¢ç¥s?ŠoԖ#°?w.Œs-G!?ŠoԖ#±?ïšï/6L?¨þ
só¯ ?‰42mB?¨þ
só¯ ?îdÈçž}?²šÜ(1Þ?©³q†/Ç?²šÜ(1Û?ïÿÿþ…Vi>a"5ٙå~>'ª™iAí'>a"5ٙXÀ3FGL J1031.0+7440@`ǗͅY@CšÀ ýÀ:&sÔ
2îÀ;´¦ÏB.À!͋¹‡ @M†ÇÚʑ@,"ß}ÿ_¿ÎY 
ý¿ç¥b•ÿä°¿Ü[z"0t¿äSr€'TAGNbcuS5 1027+74?ïñOÛè_?lU~ƯÎ?]`IÆ/A"?lU~ƯÌ?ï©'n'¤?¥gùq…M×?…¹ßd[–ü?¥gùq…M×?îgåÓl{é?·•l½"E?©¢É8AX?·•l½"G?ïÿÿú—}æ>ê ®á5€>E¢f>ê ®á°	3FGL J1159.6-0723@q'Êßø"¼@J¢€dÀ9Ҙ×ÒºMÀ;¢Òhî#À!͋¹‡ @x†ä'@Ôɀ'±¿æQ:›:G¿Ør‰ñ¹t¿æð±$´|¿¯ƒ-–mžAGNbcuPMN J1159-0723?ïvŽÕÞ|î?›"J}îmž?'.%D0bA?›"J}îmž?ï½ëÉÜßÉ?™Ä˜­ˆsà?€…
ˆÈ
Ñ?™Ä˜­ˆsá?íéžû:? …éU¾½?°³Ð'.? …éU¾½?ïÿÿý—æ‡>kµæqP >3@Ë̍ëù>kµæqå3FGL J1832.4-5659@u#–Óõ¶À4¯ÿ6¬dÀ9>ô×­Ñ_À;–Ë1ÂëÀ!͋¹‡ @´:¹ºKk@'¾Ÿã_¶¿é!á+ ±¿Ù
¨4¼ö¿è­·ŸOLU¿â.e-"ÅIAGNbllPMN J1832-5659?ìó$§MK?º^Žy¹?¸fÚœõª?º^Žy¹?ïº| N!?ª	FR¨6"?`×ì[÷Á?ª	FR¨6"?ëù™æ ›‹?¦xâ"{?À˜g}'Ó?¦xâ"{?ïÿÿù¨u>Ñr¸‹N >K^/Ï>Ñr¸‹H3FGL J2358.3-2853@5H€_5ð}ÀSŠ« ,ZÒÀ:GpJ붝À;õxZ"±À!͋¹‡ @žIaÈÈ@OãÀYK÷¿ßÐ¥æ?JÕ¿ê®tŒóe¿ÊTLªË¿ïÿ'£+ÓAGNbcuPMN J2358-2853?ïãüZžî'?"­ý'ƒJ£?l¥amœ?"­ý'ƒJ¤?ïìNîbù1?'\ŸÉؕ
?c±λ?'\ŸÉؕ
?í£À}š×á?¤*™4ñ¤ƒ?²áü)@ò?¤*™4ñ¤ƒ?ïÿÿþ°aF>\‡aíÈÞÐ>$ùë¨mŒ*>\‡aíÌ÷Œ3FGL J0534.5+2201i@g´ßݵÀö@8ªAÀ5¨†¡oPñÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ú=p¡'Øa¿Ó×o9ìh¿Ù3Ší•€l¿ÍÉB˜o¼À¿ÍЁ~+^OTHERPWNCrab?ìVŽmx"?ÇY™SZÃ7?¿}KŒ";d?ÇY™SZÃ7?'&«"¿5?°Ã/ÀÇ k?ï·eQ±+?°Ã/ÀÇ j?ë4¶ð˒?¯þ~¨*Ô?Ã-'œ<Ѷ?¯þ~¨*Õ?º¯ßô‹?ÓsÂ?!O¿?ìª~Ž?ÓsÂ?!O¾3FGL J0833.1-4511e@puR}ÔAÀØðߦ™1À6!vu¨"ÉÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@G̀&¿äqªé3q¿æe¥åþ™¿äqªí~óü¿ä§ÍP¢§,OTHERPWNVela X?íZ‹6,?Á€­b–?µ/S¦NŸ¢?Á€­b–?'|iaU?°ÂáƉ¤?ï·¢[ª{?°ÂáƉ¤?èÉ©{¼Ç?±˜h"1?ÌÙZùã?±˜h"1?»"ÔæçÒ?ӔlÐd?ìž-…c#?ӔlÐd3FGL J1514.0-5915e@tQ¿zÔ²¿ôWõÀjÀ7Ï{-ÇýÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ù$5½À¿Ñn£ Öå¿×!ƒït~¿Ñn¶t¤J¿Ð…[/aӖOTHERPWNMSH 15-52?î˜Rñw?½>:4¬¡ú?®æzÐ?½>:4¬¡ù?€"/t]Š?¯ù/ùÝ3?ï½³B.‰×?¯ù/ùÝ3?ëw{äDás?®g´¤f<?Â"nìz7?®g´¤f<?»?_dÇßî?Ӟ D¤˜?ì˜g?Ӟ D¤˜3FGL J2021.0+4031e@Sp¿ñ7@'˜à66À92šs´-Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?øzá? ~æ¿Ð&
ŒT¸¿Õ¨xöræ¿Ð&
±Õ‹É¿¾pç&räOTHERSNRGamma Cygni?쯳¿«ß?ÅSîVo8?º'b¡ô?ÅSîVo8?€u¤RÇÿ?°i®99°.?ï¾+­n´à?°i®99°.?ët>Kà ?°¹U{žô?Â/Óì}ƒ?°¹U{žô?»Î£R^nÌ?Ó¿T²?ì†+•´2'?Ó¿T±3FGL J2028.6+4110e@Sæy€žQ?öVŽà3·À5$‹
Š}Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@ff_°iÀ¿á¸•Ý0r¿ãêáF›3¼¿Ê²ôQ©ž}¿ãÊ­" ®¡OTHERSFRCygnus Cocoon?íüÊÛÊr7?¿@=¢jiQ?°©!¬nE?¿@=¢jiP?F"ÖÑø?°¾,ñ±ü?ïºçwø¤¸?°¾,ñ±ü?êæâ¾?¯)¼ÑO?Äe‹»¨u?¯)¼ÑP?ºÁøÚNî?Ó}D;…è?ì§Àþ¶#?Ó}D;…é3FGL J1513.9-5908@t#àz(»¿ò—™:À7Ó%ô†O:À9ø˜˜—;À!͋¹‡ @d<˜â'@óƒÀig"¿ìÆ¿u)¿ìž=e^¿áÃn/Ĥñ¿ÒºTûPSRPSRPSR J1513-5908?éC®Ȓ"?ËfMT½õn?ÊñG Ýµ®?ËfMT½õn?ï‡cSŠ÷?±íòÝáo¦?Ž'+B:Æ?±íòÝáo¦?äWv'ࢼ?¶Vb1D«:?×Qú>º‡?¶Vb1D«:?ïÿÿÿí¡f>FÁß}b=â^™lrÑ>FÁߊeJ3FGL J0121.8-3917@qU{à~íÀSË¿ñò÷À:¾8äMÀ;ÿÍ2MZ&À!͋¹‡ @èw9@?üÊb&%Ú?ïôöŽ®¿á°ãôAí¿âO²vE'¿ã2ã#žUNASNone?ïþâøË|¢?1çã
¶?!ÐsH5è\?1çã
¶?ïð}ߦQ
?Š°}a›x?_@³]ê|?Š°}a›x?î$îgÏP? X†´‰F?­±ƒJþ? X†´‰F?ïÿÿþû·?>['F"¸Ã> DŒ'ý>['FŽØê3FGL J1655.1-3954@u',à2Û@ÿ8x[0À:fÿš6À;â1¸ß°À!͋¹‡ @;,‡óSõ?úàåáâ"?ìºvçpš¥¿çIÕ·¿ÔuÌX2¿ã'?™UNASNone?ïîºÜ¡zÛ?|¬jû¸?aE#^…$?|¬jû¸?ïÚæ¤íî?À5ý[]œå?œD£+bBJ?À5ý[]œå?íôÚÀ?®"'ùÍíú?·h_‰)ÿÆ?®"'ùÍíú?ïÿÿò¬'>›™
©ß>[ú¦ÜQ°æ>›™
™¹

==> SOM_VIZIER/3FGL_prob_catalog_3classes <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  509 / width of table in bytes                        NAXIS2  =                 3034 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   65 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\3FGL_prob_catalog_3...'TTYPE1  = 'Source_Name_3FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON    '           / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Signif_Curve)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'ln(Variability_Index)' / label for column 7                          TFORM7  = 'D       '           / format for column 7                            TTYPE8  = '500MeV_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'HR12    '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'HR23    '           / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'HR34    '           / label for column 11                            TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR45    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'Category_3FGL'      / label for column 13                            TFORM13 = '5A      '           / format for column 13                           TTYPE14 = 'CLASS_3FGL'         / label for column 14                            TFORM14 = '5A      '           / format for column 14                           TTYPE15 = 'Flags_3FGL'         / label for column 15                            TFORM15 = 'I       '           / format for column 15                           TTYPE16 = 'AGN_BDT_O'          / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'AGN_BDT_STD_O'      / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'PSR_BDT_O'          / label for column 18                            TFORM18 = 'D       '           / format for column 18                           TTYPE19 = 'PSR_BDT_STD_O'      / label for column 19                            TFORM19 = 'D       '           / format for column 19                           TTYPE20 = 'OTHER_BDT_O'        / label for column 20                            TFORM20 = 'D       '           / format for column 20                           TTYPE21 = 'OTHER_BDT_STD_O'    / label for column 21                            TFORM21 = 'D       '           / format for column 21                           TTYPE22 = 'AGN_NN_O'           / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_NN_STD_O'       / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'PSR_NN_O'           / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_NN_STD_O'       / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'OTHER_NN_O'         / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'OTHER_NN_STD_O'     / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'AGN_RF_O'           / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'AGN_RF_STD_O'       / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'PSR_RF_O'           / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'PSR_RF_STD_O'       / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'OTHER_RF_O'         / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'OTHER_RF_STD_O'     / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'AGN_LR_O'           / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_LR_STD_O'       / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'PSR_LR_O'           / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_LR_STD_O'       / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'OTHER_LR_O'         / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'OTHER_LR_STD_O'     / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'AGN_BDT '           / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'AGN_BDT_STD'        / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'PSR_BDT '           / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'PSR_BDT_STD'        / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'OTHER_BDT'          / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'OTHER_BDT_STD'      / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'AGN_NN  '           / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'AGN_NN_STD'         / label for column 47                            TFORM47 = 'D       '           / format for column 47                           TTYPE48 = 'PSR_NN  '           / label for column 48                            TFORM48 = 'D       '           / format for column 48                           TTYPE49 = 'PSR_NN_STD'         / label for column 49                            TFORM49 = 'D       '           / format for column 49                           TTYPE50 = 'OTHER_NN'           / label for column 50                            TFORM50 = 'D       '           / format for column 50                           TTYPE51 = 'OTHER_NN_STD'       / label for column 51                            TFORM51 = 'D       '           / format for column 51                           TTYPE52 = 'AGN_RF  '           / label for column 52                            TFORM52 = 'D       '           / format for column 52                           TTYPE53 = 'AGN_RF_STD'         / label for column 53                            TFORM53 = 'D       '           / format for column 53                           TTYPE54 = 'PSR_RF  '           / label for column 54                            TFORM54 = 'D       '           / format for column 54                           TTYPE55 = 'PSR_RF_STD'         / label for column 55                            TFORM55 = 'D       '           / format for column 55                           TTYPE56 = 'OTHER_RF'           / label for column 56                            TFORM56 = 'D       '           / format for column 56                           TTYPE57 = 'OTHER_RF_STD'       / label for column 57                            TFORM57 = 'D       '           / format for column 57                           TTYPE58 = 'AGN_LR  '           / label for column 58                            TFORM58 = 'D       '           / format for column 58                           TTYPE59 = 'AGN_LR_STD'         / label for column 59                            TFORM59 = 'D       '           / format for column 59                           TTYPE60 = 'PSR_LR  '           / label for column 60                            TFORM60 = 'D       '           / format for column 60                           TTYPE61 = 'PSR_LR_STD'         / label for column 61                            TFORM61 = 'D       '           / format for column 61                           TTYPE62 = 'OTHER_LR'           / label for column 62                            TFORM62 = 'D       '           / format for column 62                           TTYPE63 = 'OTHER_LR_STD'       / label for column 63                            TFORM63 = 'D       '           / format for column 63                           TTYPE64 = 'Missing_Values_Flag' / label for column 64                           TFORM64 = 'I       '           / format for column 64                           TTYPE65 = 'Category_Prob'      / label for column 65                            TFORM65 = '5A      '           / format for column 65                           DATE-HDU= '2022-01-29T22:22:37' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                             3FGL J0001.0+6314@]RÂÀð ?íŸWÿÎàVÀ9ZzŸÙOÀ:ÿ!Z³¿õÆkvñxÿ@Å "	¸@ܾßú&!¿ç0WìPӿ쳊Ügu¿ÜƒûÂكê¿îæý/k'–OTHERspp?êʕœMÂÅ?Á+ɋ¾~o?˜­ãx{`?™y	œ¯û:?ÁÀòß>?ÀÁ zD¥Þ?Ö>rƒ¢ƒÅ?Ö»ק'?©ÕQ
¨K?«>Sš€Û?ãCq­¨€x?ÖBÛh=?ä­y΀´¤?¶'Í+Ù¨?À{1#¹mŸ?¥ýÅío?ÌÎç þT?²§5yvó?ë¶Îpq[?²F|Ûm°z?mO62,@?sñq™ÈÑ?À¯‰gi¾?²§²¬¨$?í×ù¢T†?²ÿk'º?‹?®Ô"Ë-?ˆ°×»Í§ç?«°z&yËÐ?²?-΀'H?ÝљHC™;?Ù×ýƒñ3?­cé6{ê?­KïՔ?ށé'K
è?×ÌñÆÆ?éŒ;ú¦?®p|lqŸ(?¶ï)Z¹¬V? ûÃ8ÝÖ?¼®þcPdû?§7°àüèE?îzk²ðF"?•ïâU¿?K=;…3?F»Å´ÆÃä?§ìOáút?•Î""'à\MIXED3FGL J0001.2-0748@VAk¿×ÀPÔÀ€"ÐÀ9"ñóÍÃÀ;¯Þ>Xˆ?ä‹|¸&;@Avû	 @1݀#Pè¿ÔÇZö#eé¿ã+ùÖζå¿Û5šÜdÅR¿í›Q÷æÎAGNbll?îmsmWi?ª_^Uèî*?ª8A÷ÝvÝ?©7ÀÓÈ©"?€›J[´U?x#w܌Ã?êûÔK¾'Ã?½ÌÃßà?±áM~Õ?±:Á¡—â?·|T?±)©ûCü?èS•£ë­
?°Œî"þ?ÇÄ:¤c¡?¬l¹_ßC?«µ»-%¶?•Ö5eÄSL?èKœ·—lª?°ßzk¯?±õ*3y6õ?£:ӄ"±?ÅÖø@ğ?ª""D#u?ï×;ï"?ŒrÂÿ¿I?™8IóiÈ?›æ5G˜A–?tl–sÏÑ?j÷;Hõú?í–ÿ{­?¬	EÔï‡Â?£o9=¡;É?¡¼óµ7?£ ֑×	e?š,d[ ‰?ê¼íi$†È?ªˆŒÊû ?À­UzÓ'Q?§†áür\?¡{ӆ¶y5?ž{Y&\Â?ímDY©È?˜zþ|[ëð?¦&ç»ß–?‹'J»q"?©=Ðñµê?'?-cü®ÜAGN3FGL J0001.4+2120@Zê–_RuïÀD	@¢CÀ9‹!P²ŸûÀ;ÎÑPÀô?÷ÁF#zÙe@{J¨š¾@d´¢´uh¿ã©OºÛç%¿êJJAuHà¿ïÿ:ÕÇ?º{	¥_rAGNfsrq?ïóÞ|«)í?[f2Ù
?7×åÁ4T¸?;Ú³H:q?RM
Wáþ4?WU©êœƒë?ïz›	0U]?•F$Ÿn?kŸâPu?[Œ»¶4?ŠqE—œ?ŒkÛÒ@''?í_ÅU'·0?¡Ç4í?—?¢¨,̕.?—3ëŸ2Ñ2?§'wtB×?šPzñØ?ïrðF	à»?–Ú4ø–?pë™6?ƒdš'÷–µ?‹<ëøôäg?'¹œ¹÷—ƒ?ïú¿ØXØE?J¦o‰˜Ñ?*7zz­=–?5À¡2À
"?<åŒÚCÛ?BïXã>jA?ïÙÒ¥'Ê?l;×n×?Rf¸G6ü¾?Q"y‡?vÑ?lùÿ,"?f£J‡¾s?îx,®×é?—]]´@X?˜ƒ²8®?ŽÛ	'^	c?˜v¸
k&?¾ú2Ræì?ïë(á…t?sz£ڐê?QšwHä…Þ?h–Lù|?XM
·?d–þ$VÎ"AGN3FGL J0002.2-4152@tá !¸ÀR	"`¸À:†¾š§·À<˜¡L'¿ùº­ Œ§ï@ \2°@¶ÆCò¿éÖ%8ý*@¿çž>éí‡?±Dņ YÖ¿â"yq…ÿ3AGNbcu?ïý
Ünç?-Z£¸u¯?ëg'aâÇ?˜Ž9—º3?5kŠ–]+?+G;ƒ§s?里ö‰	?ƒimJ'?b"#Ÿ× ?ewÉ)È?ºðnó?€?í¨b¿?ï'8m|&¹?'³¬iØw?}¿Ò E[.?g¶èWjf¥?"¨ýÊ! ?€SΈ2™Ó?ïÚaB?oï҄Ëm>æ9T¹>ý¹UÍðö?rÄBS Z?oàÕÓºî?ïýÖô²³¶?(%·»¡*?Âã?5¢>öÑ#÷*»?-ŸþS7[-?&çˀµÎ?ï᝔P£?iðÞָԊ?NÕy$Å?P:ç1ÿãÅ?f­&Žgô?c›.
1?ïžNKßÉÌ?m¯ÃAÕ­²?q"&+ˆ?U–ü§J"3?¶³ÿO?iše•‡?ïú\ݦŽË?;y`éªù>Õ@Ä#çĈ>×¥å¯Ô®?Fb]džg?;TA-A`®AGN3FGL J0003.2-5246@sïž?»×²ÀOiÿ¼ä!À:‡¯»DMÀ;èK	éÎ¿¸otpl@€Ä©Ü¡?þRÅ؈B¿ïýñ$yœ?ﶰÅýr)¿ÙjÓ³'	¿Ý¾_îõcAGNbcu?ï÷A] ø'?HS=x½ÿþ?ÆÝ"Lb?uBÀ¸?OA­Î§n©?FéÍÉ^?ïo‡7þZJ?Éÿ¢hôV?oN{'åKÒ?y%qþná?ŒJ"'Ò´?Š­:˜ÿ¬"?ïE]_à?'µ'[Ñ?ƒŸg–iœÒ?pJmï[?" ƒ#ӝ?~螋.»?ï/Å?öÌ?""Ÿ[YÖ?}»cåÍåª?xÍ<Տ'H?'®®Zš ?'ƒ6݋½?ïúñ#r7?9=ˆÊvm?b›y?"Ö?ãí$%
?AÏsâ†?7wª¦¶–Ñ?ïӊ,Øê×?uZŒ6`R?U½%OCÙÏ?Z؈=?Æ?pË 8*z
?pŠiPRµ#?å"nâ?s¥prÇÞR?wk«b*Î?gñ|<c
?'°í–™|?l8;öpH3?ïÑÞ p¸?m¡""°?]Öj¥¦Ea?RûNu?o6*}¼Í0?i"ÕXÇ]AGN3FGL J0003.8-1151@U¤ YÀQÅcÿï9À:¬"V;uøÀ;ù è­Óã?âŸ8ÅCk@
¢'<@0+ÿ>l?éyÑyý‰¿ØóK^¿åD:Ï<q¿Ü¼ûßðýAGNbcu?ïô-Ð?Q]s®7ˆE?E»N"Ù$?E<ñ?ú¯?Iëúm!Ÿ?G{7­?ïY?ï\º˜‡¡?"Ûtš¨º?qsÊ:hâ
?|§§`à?Ê 'a?ßv³ëž?î´?#ù¦Â?rÛôðÈÏ?"X~fûF9?ƒ2 >.þâ?–ð©"?€‡F!κ?íR= ° ?©ìGʤ?ÛÙBŸ?Û=ðÿƚ?³wÂtÓ=?§U'ºKR?ïú4e¢9?A5Aš?2»²/Å]c?2à'´RtJ?;¡%o
Ã?5©	pkP¤?ïÍ-/ìŠ`?u`:!îÎ?ZÆJh¸2?[Ò±(¬ø?r·Õp웄?p"L ­)?ï^Ã8"3=?}s˘1'?…ê)ʖÌ?w˜¢BÉtò?'e²Ê¤?k¡1<‡Ë‰?ïNtuÙÝ?‹
´`…¬?zätèp?r|`Âó8&?ŽðÚUóèË?†#‰($ÁAGN3FGL J0004.7-4740@t=Ÿ¶MÀPá1ÔÌvÀ9iÎ,H]gÀ;؂—õT«?ãqP7®u§@è<Vžó@:f¿§ C¿áMwé+ä¿æXÜZ½³¿äXzLnºë¿ïÿð¸å9UAGNfsrq?﹌¶‡;?''}`늣?p€ò¤è-?wé¦4®R?r¸²'sÑ"?wY¶F¤ÝK?îÇÉÔ*(?ŸDXÆHW?ƒ±3",i?"@spa¨?.F#ËÀ?˜±¡Ìc³h?í†o39?ŸK»Whùg?¦MØ÷Ž¨‹?–ïCø°Þã?¡Qªnï?"Äv½T<?íÈñ
ûm?£ýjŠž5?""öÚvàZ?òԋlŒ?©¦ó…"u? (0
Îo›?ïÎjµð+;?|ÝP»ãÉ?l^˜5?uZò"ì?e7Eh¡Ht?jrôIT'	?=÷¡?†$½úvÿ?uqô#$á?ss=×HË?ƒ"?'ª3[?}N•Ã*÷w?íäaŽQ?¡ú—é^?£4$H¨ž?—¶wŒ-¿9?™ìCÃK?•–Oùl±è?ï'èQ¯íe?'£ø{§ð7?yÕ"çú?p=l–ï'?'ÂPYY?~•€ÐŠõAGN3FGL J0006.4+3825@\U=žÇÀ7‹@;À9Jn¿Ñ;ÇÀ;™2"Ѽ?êXyç¼V@&í @ïဎæ¿çGkÚ¢+¿æÝH
1ÿìNC–œ}é¿äz"&V½AGNfsrq?ïö‡ƒ—y¯?NlÍQS¥?FSÛH<@í?Hz½Se??+º#68?:^Åî¼wì?îtcèT?¯pà´Ê?‰|«òî'Ç?'íÀœm[?¢_nÌý¤O?«lBš?îµ`˜Ø:?'ùÄ9›Ñ?'ÏÏ2C#_?†îǎîq˜?—Äº¡Õg?‡í1äW?ìˆb@«°Œ?§èÌjxÛ
?¢}¡Ga39?šst8Xƒq?²~U:?£ÜSkv–k?ïú|ß_ݜ?CÒºøcÿY?9Ö>×tc?>¬$ªÆÒ¿?2BÆzû¥r?0+œNÔ#?ïŠúâß³¯?'õc~[xí?q@^'õ/Ì?sq'=7?"¡5xTG?C9D}?ïW‹ÇôËÄ?"£9éKVÂ?"èWí§¸Á?€Â¨{õœâ?…4¶µº+?w†²IÞWN?ï.[¦!šã?‰³6L
ç?ˆçÞÞãŸ?s›«Ñ¯Q"?ŒY.•JǨ?…r}×ä[AGN3FGL J0007.0+7302@]ê_á'p@$ëÎ ‰ãCÀ5"á÷|þÀ:H!ß&¡@ö%/Íù@¨Œá¥Kÿ?øè!¼é)û¿É_:@KRA¿ÙyB+s¡7¿à掝¿êwë1olRPSRPSR?`Ïå¬$à,?jGž.ð?î/¬k'f?¶\Ɂ>?«ø:ð´?¶qá[߁?K'~Èåã?ižed==?îz ^‰%?¦Å0^23†?§ñ\ªr§?¦Ã«žùõ?­"Û%èãR?¦ß6žM?çHzº}·?½\'·‰)ñ?Ì5§L	ÃÎ?¸*xIsٚ?Bf±DÆ?Pâ#ó8•?î· X˜¦?žˆ¥@Hù?¤EˆÜn;®?ž3›dª6?S^×c.?aWx°=?íÉXÛõ?¼;Ä"Ž?±–<'Ý‹×?¼¾Ù6]?^w]A•Ú?{/4Ëäšt?î+ÜÚP?ªÈo4µ!1?¬Zc"H"¹?©Ïx7N?µ`H"È	?¥"ãÖÃÑ?äød
Ÿñ?¶<QÝâT?з%ÉÆ»™?´Mf·Bl¤?FW>9Ò4?A83Œ&×{?îìCQ°Ä%?'!z–Lœ·? ân"ùì™?ô¯×ÑfPSR3FGL J0008.0+4713@\ÕH˒:À.WÊÆbÀ8‹e²€gÀ;<µgUy¯?íñvi,®@Ó=…Ï@+?ëÓM¿ÀvþF
ø³¿àœ €Ò[¿Ú̀èYˆ¿äC9qzAGNbll?ì>YqœŒ?´u¶2f
Ÿ?¤\\=SÚ? —jLR?³á¿z33?¯Üfoa?ہp*èêm?ÎRvÁ
¸?×)ñ¥
/?ÉS˜Áµõù?Ê©<]î¦?Âqmd¡.'?êd×,n•V?©b	¼?¬€?²vX¹äð?›:žõ>ª?º¼ÐD?cÝ?¢§óä
½?ÕÃ5öBM>?¶ªœë‰À?ÐYª $©?ºn)5Oåh?Ùãé™%?º¿²"?íр"cI¦?§¡!ƒuz\?›ã?duɦ?˜Ý¿4õm?¤öWlgÅ?žèÝð"Ì»?åóö@¨?Ë>=ABÚ4?ÈÄzòÿ*\?Áh‹Qh?¾Þi'O¦?¼ò¦N³Â?íX¹£‹q?ž­8¹®,¼?¤¼æ±Â‰?'jñ)gFO?¦b¨äǒ?"q©gLRZ?â~ëîù?¯
ljë?Êï,"Sr?§c©3õ¸Å?Ë'ð~?¨î¢ë"ósMIXED3FGL J0008.6-2340@I#ڿԖÆÀSð*ùš‹À:c)ÒaaDÀ;¯S;ç6Û¿Äû¢£-—@ÜAƆb?ù•<@5? °ò?'Õ?ïüz¨£Þӿ窜>öœ?Ú£¤6¢ö²AGNbll?ï¶u~(Ç?¦ð±ö‹ Ö?J¯DIºt¿?SJ‹/n»ž?€Í®\fã°?¦ëó¶Ig?ï›WËݨV?ŠG£þX}H?d@øK_Õ?vŒ"kÁó?"Îë…~•?ƒþˆáWt¹?îÜÛä?–ukÊ¥ìh?›8X@/†?‹üâeћ2? ãkEÞÿ?8 
•
?ï‡Á¯&7'?éÁ)t{O?Uõã‹D,?o/öàÃ	
?‹P×µ"]0?2°ÜuD?ï°m¯õ•]?¨L¿omÖZ?Hõ)•¦«?2šw˜?'UAd÷?¨õ*±?ïâ.>4v³?jW.8–'?L¯.7À–?PSnÈ<5$?f¥ö]åšk?dS˜xTß?î·NõÜC?"£ˆÌ;A?'ÙÒÂi£?‡"¤b+‹x?–=(Ç¢Õþ?Ìôµ=?ïìÎ05c?b'·;'Åg?U¹hqÀ?"pìØ1îæ?b7'qф
?b@šõAGN3FGL J0009.1+0630@ZMa²¢ÀKlR@>´qÀ9Íêï̓À;µþÓ°Ý¿ïæJ˪@w"²î'@oV@S'3¿àmíóQá¿ã-˜û¿áW¹aÏÿàŒ*h¼àyAGNbll?ïé³ÚHÈ?`Âõ¼¼Õ¥?4Ä?2 ç?1xÀ»ÔÁ?daÄ|¯p¡?_u°~(?ï'`<šÕ?‡…]?* ?d¤½;ð©?r\R"G?†~É­Ô'?¾>ò]šÛ?îÞѕ'M?¤ü4Ÿ¯?‰Ã>"Ìf‡?|ƍ›D º?—D.My?…x)?;®?ï<Ánl;µ?‰<Mÿ‹g²?2ä'-»,?2mÿЪkw?˜?í$û?‰¼>>?ï÷1ó9X?K3ÄkV`?%ù?ñ?"±–êK´?M¹ò*?H§|nRÝ?ïÝv_¥#ˆ?i(8Äô¼'?PTЇ	X}?PCnX€j?j_8<
?c2¢ƒfì?ï'BׄÐy?|ÞR•ªõØ?yÖK(ÚÙ?zžid	¯?}ˆIþz°?e¸²¹mx?ïØþC'Pû?ai㞝K?[Ud/î?®{á\~w?s+q­HKi?aE\<9 AGN3FGL J0009.3+5030@]s`Iì³À'›I ÛAÛÀ8ҍÖí¸À:ú€ÌC:?èNêj±="@e鋁 ?þÛ°àˆŽ¿á"¢x1¿Þ&úÓùÅ\¿Ù͹"¤³¿âQ®Ñí§AGNbll?ïôꌢ²?VȲåÞª?"­—øaª…?&ì|ŽW>
?SÕ5nÿ>?TƒaÛãþ?î"ÆåÆݎ?¯—^YfH•?†š×Z'?‰º_Ö?¢ÛÍÊy?¬4õ±µ?î<Aë‹—?›0?]Äôj?Áƒº×yF?†Ü9—ÊcE?£ÛsSWî?–<Ãiq"µ?êÇ£ ðª;?©@}4?Šw
j¥T?Ÿ¿­Q?Ã:Û&¬½?©E´´
Ò?ïûèQɲw?9{@-ºÀ?šõÌÎÏ?@tçBŒñ?;–µ»1
?6pøgÎ3¦?ïXDœ?že(|4©·?uTë+.?wn®Ìð(?DðDØ€?™9"lG??ïN*',?‰…ü´N?€1 ýÝ+6?xó]hù?ŒD>oè \?"òEx¡O?î!Ψ³×¢?NÅGä?ƒÅe7mÃ?nþ.uÐd?¨ñ¼¼Üo?ŒÑkX#êAGN3FGL J0009.6-3211?ôÒÆ>¾ÀS愠
Q!À:iÁµA•ÍÀ<YQªí?›¹ÉŽ©H@™ÎØÿ@zSŸd^Ͽ〠ƒ¿ãô](5dw¿æ¶"Ò
¿äbzª¨hAGNbcu?ïoñÒ7<O?Žpk?Y€àWɋ"?U½rNÂ~í?i·µ«¡n?ŒØ¼ð
êj?ïMãm«³?"¿ÛÙ¢K®?u([¯?}	k»?'ÿ,ø.ñ?Žñ¬QÃqM?톊‡Ð;?šžK5CÚ?œ¯³ŽÁ?‡ڀO×À?©"|à	ò?"ÎÁÕ´
?íȽr€"Õ?ž=ƒØ·ó"?ƒ2LÀ]?zã«9já÷?®®FRaÜ?œP8†í
(?ïÝ8/Fiœ?r¦—iu²Ý??KnŽ­Ê?>f;œƒñÌ?nÞ`vvú"?q…œo¶i?ïÉÎ-2?y4kXôÑä?^¢Ímñ?dè¤/{îæ?sÈe¯Oi?q6ÔY\]f?ï/0ô@j?€T¦Ö²?†'¹4<é-?tZ \ê?±CŽ²ü:?sÌ즶—?ïŒIBáæ?y©¥rACH?iyÙ¶\?V;¸SHEw?†gvÊß?vòëûªEAGN3FGL J0012.4+7040@]ëþ?5Ÿõ@ Ì <ÁÀ9Ê ™ÙZÀ;KÀæå|Ç¿ù¦®ÕëÚ@‹`Þj.@Þ¸@xÁ¿ã
Q2L®¿ëÓP¹?
¿â1Àª³%¿ÜGÐç—1AGNbcu?ï¼Lë|K'?'1G!F^?@ÑW^SM?7P.*¡ð?ÙüÑe!?Ý¦¯ÆÈw?î5D½Ê%~?¸§Ü§ôà?}#Ìáèì?‰Š¡FÍ?©:¢ak	?·˜'h?í2<¡›ò?£0a4C?"7ªƒz2?<èÁ"ß?±¡3y8¬î?¡¶és'?ï&çžÆef?‹¯"Äub?èa­E?8ÜÍ?›CÃ?‹¤µ©!œ?ïò:()G?\³F8Õ{Ë?,d"t°<6?$Õ|!p­?WÿKxÇ
š?[=ÐýªV}?ÜA½?•ËACð?a°
Ǽ^??fÈÆìW¾m?‡³t×°e?"·Òe˜?ï"4{eYª?ˆqœžˆv?~«‹Œ£*?húY2+bc?"«\Œ3?†ܘ.Ðò?ïÏèDÄÍq?cÛülVþ/?$°ÔHQz>ûÂź¯n›?wç"\lŠ;?cË;©Ÿ¤AGN3FGL J0013.2-3954@tÅ.@…+NÀR½"@(äüÀ9¯ó¢#«×À;ÛÞ|!¹Ž¿þ)
Ðx(@¿(Ÿ[z@±»€Hj¿â4¨©,	¿ä+P)§Þ¿â¹).<¿Ös³Èç1tAGNbll?ïØTŒÁ'R?pÚã"ë
§?;2"fh&
?:(b.¹?r"\ÞÅ?o]…(o÷?狀f˜»M?"ŀù?bT˜JqÁ?dW+¸¦]?|@L´)6?€>Z÷S™?œ‡›Ñ?¨köFŽ?Œ¦íõNf¹?wÖz³ÿ?žUyŒ¼o?ˆVÍò/ÀŠ?ï§I6Õª?'z²»¹?Þ
˜àŠ§?ò‰‰r?†#·s˜U?'x
×`*ã?ïóEYGçB?\[®×5]?.¸Ê¯–ƒá?+8ý¹ßù:?Už4›)œö?YíüþÞäÈ?ï↙¦sŒ?ixäZAD?L]]`Ëðn?N⯠¿9?fbçÉ-S?cº
ÆÔȔ?ïÇŸ€'G?sŽV*h8@?w÷IKÆ ?]ÝI"e+¸?ƒ'ss3æ!?núÕjyó?ïòTÐU²(?QÉqޟŸ >ÙBzæCˆ>ڕ½2É×$?[=¸ià¼?QĈ$AGN3FGL J0013.9-1853@R¨øäÀS…€,á
À:¢ÐqœûNÀ;þ¦Ë±CÚ?ß!0wþ$š@Äû—»s?þö`¾ø?ïøÀá\%ñ?Õæ/–½é|¿ÚëlÌVo¿êǦ—}"AGNbll?î—"Ì¿?¨ô>g@?¢œÈ°Û?¤¬1B_yw?€6ßû`Þ?‡Ñ暱Ð?æÚԟÉ?Ì0°U¸?÷:`Æ`Ä?Ãã3Û=˜?Àà¾L½"?½[š£kì?ë\OÑú^+?¨F•<Çï?¸ÀOL)µl?¤}Z!HIý?¨ºdLR5y?–}Zûw{?æQ›ºAk?Ãv±8áb?Ë&oÒ-Ó?Á¾8;9x?¸à"z±ý?°
Y!XÅ?îlñ_.ö?´§²!íéè?£,YP-ˆÝ?°uQŸ[¯¼?ˆV™¿¯-?–žaéú¼?ë{FUW}ô?¼†ÿ>JO?´ˆK®‹5?³•ø[c,?¯;Pj½?§ßL«O/°?í8Šò%?¡š
¦~?±Ñ$Ô®j"?Ÿáê@P'5?˜"[Fk¬ô?Š
îGtG?ìøŸm»fÀ?¥ºP‹m7å?°1wi•†?? ÿ uá ? Qún}?—÷Y~¦˜AGN3FGL J0014.0-5025@s×7À*ýÛÀPh"  0øÀ:™û3èdÙÀ<0{ÈÎ;?×Ɵw»3®@±Ëžðñ?þÈ3€5'¿ç§vóÁ.¿ÑÔ'54P{¿ä/çP~$¿ÜºhÆïƒAGNbll?ïì#¤A_¾?\tFg²/¬?F.ƒ´|g?P©ß£C?\¡u3õW0?Vì+ÈìԐ?ïfB:sT?'¨|æy~ï?n‹¯Ư?s­åJ®å/?ŽÌ¯³›Õ1?$E¨­h?îӕÎUZr?‡?/q°è?Œ~•‰XÖ?wÓ{-à?—Mû±GÓW?€è$êäœ?î‹»ÎÍ®?–oe%)Ö?}9¯%Sjñ?zA1TŠ¨?£§~bL>?•vI"ï™?ï÷€'ò}?RøjbÞíB?7Ǭ"•?Q8¾i
?FÈ©kº‰??‰—F³%?ïÓÇ*ªM?sgó³Pã?V¬ÆW ?W÷5ƒ?p™bÃ=ß¹?müE"6˜ã?ïx"†x«?sñ2äÚÜ?}}Yì¶DF?h£Ï¶2ÂÐ?ƒ K wE?jlí¦ý~r?ïªkÔâ?t"¢O›×¶?hm┳Îs?[½×Gá~?~",øóz˜?px‹_ú¦wAGN3FGL J0014.6+6119@]¡ñ'l¿óÑ=ŸÈ²·À9"=ëóفÀ;QÙ($â8?ìqÌ[ã¬@k¾vçÂ?þ3#Þ¬s;?î'NË®Ùa¿µ™^'Ÿ"¿ÑÃñ)è ¿ÝWGph.#AGNbcu?ïR˜ÿžcá?@Óú!ƒ?ƒ¯'  @?~[£W·?‡ª>Ægi?†*_£I]Ñ?·c§3'ü?ÃÚÔï_?¶ƒõê
¶ˆ?¯›š
?êC\YÈ?ÆO"õ'`7?ì…$Ýã~?¢Ó'®€Ìè?£Oã\ÎË?"%ÑXŸ>Ï?².ç‰#›4?œÍÔoê"Õ?êkjo	£?±(­¨'0?¤k†Yøy6?ä¸Êac?Á7t­ÉHÖ?¯=N8›s?ï°ê€^Vš?{¿Å@ÍF?s?U7åS'?n›qÿ*{×?tKj–ß›€?p_•",ô|?Æ
mY}R?Ñ|÷ÿÍÍu?¸Q•³ãô?§G•]<?çs	î§y<?оYÌU?îR6Y{?•Ö/»É3)?'´+íÎâí?lUþŒ%?¡|ègjÄÛ?'¿¶¡­³Y?í¾˜•/?•–C-Ã?ž
ŸÔ/è\?…O…îÍ?¥Ƌ¹2ñ?'+ÛaKZ®MIXED3FGL J0014.7+5802@]"Ñ_ÄÖÀîQ`Dä6À:.[)òBÀ;'Y5%{»¿ÙN´þúÇ\@
i•ûg¿?þšåŸ¶´?퐗Ã^B?ꎽ¢ãD]¿á>Ö¿áA"HŸkAGNbll?ï欶›¢?™:>t†š?a°>¼ËBI?`	ItL7?š-"P€?˜TÒ~ã@õ?æ/¹ÓA?Ñ¢³RC?®t~ðàx1?°O÷Gz?Î"!_m›0?Íàx<q?퓛nÂÂ?™€ËûF?–¤'¢ÝÞ?'sxÅ$ ?«tCKù?•vlMŸà?봖?¸ePy°"?²ó+¯z?³¶y›+ÒÝ?®Ð;˜­?ª»ƒÆ+`?ïð³*~?}{U¡<ø?I–Z0"¼?FO߃W^ì?zôÛ4ʲ?{ñ[¡GP?ëïŒhC5?Ç$mªtՌ?š"=÷8Yƒ?¡õ ô??¹â §ò?êD¨Œ·Å?ï_ñψ?ŠÒJ©á)??…–ô—……?tq[OńÁ?"¢ÙÈل3?†¼ïÓðª
?ï.WžCï»?ŽYv˜À^?í±'R=?yœ£k×ÍÝ?'9Ÿõ-ˆ?‰mÆWߦAGN3FGL J0015.7+5552@]z,¾¤ëÝÀ˜>àŸ°À:])¦ÂwÀ;§UCÿ3?¥¼RX‹‰@

a'Ñ×@êÀ/¿ã•ÖÞ¾¿æ®ëFÏ6"¿âªƒ&:§F¿âÓ´`ÖjÁAGNbcu?{Y?¯N£jíxƒ?X¦¢ŸP?YoVbTäT?®À1ÅÚe?®Ùڄù×û?ê s~›N?ƬH'¶þ.?¢3ýÁ2ü?¨èÖg²/?Âñ2˜ê®E?Ã	ò‡œl?í·›"·¥?™âUÄ.x?•*~dÒ ?3và9B?©ñd[{$?"‡I¨!/?ëТ‹ÊgÜ? K"QßR?X\"¢?ƒp,V€ÛT?½Ø@•¾»	?Ï'ï(?ï€zÖ#Ò\?œêg´¼'?I;
RL?PüaŽà?ŽM™¨í{l?œv …Àü?î:Æèô?®÷{Pr" ?‰7Öo³£"?¾rØ>å?¦¨¹Üªò?©cð/"<?ï<
Ëh§<?~Š©?Úÿ@˜› ?j¦á&³4?"MôçN?uôË]ÿÂ?îÖå¾Fˆa?æ]Ð<YR?} £²§©?eúO£i™§?»AËVŸ?€ÿ\#'ßAGN3FGL J0016.3-0013@ZáuÑ=ÀNç…`&±EÀ9;ŸDÔEgÀ;¶QºÝ·?ó¢xËmÒ@±vÚý½@ñ]À¥w¿ã¼²Læ/¿éq`œfÂF¿í¨Âñ¤¿ÖÆQ÷!<ÄAGNfsrq?ïðH
ϐ:?f>évÝ÷&?STó÷'?cß4t¤M?HÙ 9-•d?Mƒ#£qÔ?ïÓìj±?–6lH‰¤?f?«…Å?5"Fßáõ?†;ù©¹G?7L€çH?î5^?°š?˜ÛUWž˜?•pfäHf?‹\kî_š?¡ñävq'^?'ÌN¬ô/á?ïnð'h'?›!êCQϱ?nC\¯, ?te~çiÁ?™ù'ÌôF?š5Š¡:??ï÷ӗ}pÕ?P؃P¸Bg?<ƪNzJ|?EèG'`?BNLUµüÿ?C]QmÍ?ïÞÁ=ÄÓü?gÎC})â­?PDKÃs?Nä/Ÿƒ@"?iœßBqõ?b‹ÒïÄ#&?ïœßIQ-?%cÙòŽÎ?‹÷ë5LûÍ?•#t8?ðnwòˆ?…­×•Ýà6?ïÔÇ@'p?xÔÑX˜·?Wr+`"áí?Z¨uÔZÀ?o©'Öù?t‰ÿ"³ëAGN3FGL J0017.2-0643@XêÉ`0Â@ÀQSÙÔóÀ:*V]çÀ;Ï% £y¿«NÐÅMŽ@øœJNì@íø@˜÷]? R
Œçã¿ÅrdgnàD¿æhuµ8Ü¿è¯4Ã×ßAGNbcu?ï[ã7HÍ?'`Ԛæ9Ÿ?tʋT¶~j?{é_¯±ìž?Ž¡ìŠ"}‡?'9ycè3?î3Üâ€?©ºÔýÐ
?"}œL¢&"?˜á|hMŸ°?¤`Ξtyî?¢kÄ×{x?í‡ñ3•ü?˜G[øèùB?¢-w\'ã?p"g«‹?¥€¿Z­Ò_?_tQ?éÏT'R?°ÕL²$Ó?±Bpì:÷?¤üs¬Ñ?À"^9FG¸?ªsÙJv$?ïÉØD`h\?"¡f"cú?Y'¼y¦0Â?[ÛKŠv?t¯.©Ó!÷?ƒWcóÿ–?ïq¼>pdR?"Až¡djî?z|8—Äé?‰þA3ǽ?†RÔÍ}ƒ?†ôµ"'?îì{ÿ³\—?‰ƒ!Ü>qå?'ßÃf]?'heBå,?'`DvB ?|5!=	D?îV㹬?"(Ö@n?Žo&§ª@•?N–±[?¢ûdªmŠ?'ûLÿòoóAGN3FGL J0017.6-0512@YPŠŸb0ÀP©&¿òÉ·À9)´xB0ýÀ;cî4üa?ãÂÇàÔÁŽ@Àù™´qŒ@áÀ#ñø¿äÜEZ…»¿æéú`"üb¿êvºÏý·¿àÏÀÙ5AGNFSRQ?ïüp0,ü?0‹p`ÝI?$é‡51â(?[*);'?2	½"…¾‡?(—®DÖH?ï«2C|µ?Šcüñtû?a/õ¦7z?{*QnNëŠ?€çqéOX?n-슟Ü?îåyez6?‰ýˆ"T/?‰Þß$ç`º?yd"ØÛh?–`¡ItÜ?'Àþ€­ž6?ï¦Ó
uò?óݘ*+?07qōèß?4ìÛ?i<ÿ?…ɁÌoñ?Ú¼m9Úc?ïýɽJÏ?%[Ó @+k?°Äõ?¦G¨>W?%71&±?Në«/åÑ?ïäXùZ8?i?¤yRA?L"BªúÏ_?Pu`JÀ`?dñ+†-¼?b¢›Jôšò?ïvh‡,Z?F…"¦·|?{›ÐMYS?q¸í!Ï?"Ö."ÔŽÙ?}¢Ÿ¿¸?ïï4øýyµ?\˜cvÑ$?!Ù½Ð/?xŸw¡Æ"?_uê"Äþ~?[ü4.àÝAGN3FGL J0018.4+2947@\›¨d©ÎÀ@Dߥ¥À:´Ÿê$ÌÀ;ú"#—µÀqÌMËåÇ@r÷na?ýÕ
ÁÉR?ìQ+êr,Ì¿êàƒKà^¿ÅAí§"¼¿Æ(·±TÒAGNbll?ïúENúË?Cˤؾ>þ£Ó'°>ûÚf-TÖ?Eõ¬ ?BÔ}Ïk"?ï—swy'Å?Š«M§üÔj?h¶à]j˜?}¯Ç'YçË?"t`•8+?€
&؅Šg?ïÓ¾"·?‰+gëTTõ?}"|ÁÍ
y?hX"—ZzÏ?—ÙR:ƌ?ˆ)øI\?ïê,€À?cò©cdÌ>±
kãK>ÀÌM ´ÓÚ?eÑÞê9¤Ñ?cñÌL''?ïü'g~È?4
Ä£XkC?a^…úT>úA‰Ñ3<b?9/@÷[ó)?3'Š!bc¸?ïÞÏ>þ(Ì?l!¼žòk?P
½¥ÉÅ?P+€•4Ë?i)â[-º?f^éT¢Û–?ïÇ7%tó?{Ÿ¢tïù?shló—À'?Y\Aã¼àÁ?†Yû¼&öà?zº'ß§?ïýF挎?1­hÉû>'e"¯rk>™X®Ûî‰?5Ä4t­"?1<šÒM‰AGN3FGL J0018.9-8152@sH _ñØÀA"á@!X?À9¦8‰´IHÀ;©‹K"=B¿ò½¡ÜF@ÍnkB™@š€ ¤OÖ¿å¤püÜ#¿å¡g÷¾œ¿à–hjU;ú¿Ñw-HrAGNbll?ïø¿G0ɪ?F*Ѭj?
¹6ÖÝ?å#iq$?K'R÷rìO?ElUé	ÊI?ï–úfý©Ó?‡*=ï›Î?fCÝJÇB?rú¯0t/?"°~ɚÏ`?€'Ù¢MfH?ï@‹i'OY?…A
¤X@\?zåp'þ4¥?gßa%¿?'56­6¤?'m'>|v?ïÆ¿ôû?qòÂF`]>ûèϔÚx?ùŽüds?|Ù7BÒ,œ?q–˜µ§lð?ïý:f¿bè?1†ùñ'p?¶[þ·$?Ëٍvԋ?3J±î­<;?0C3jª:?ïÜ»#Eï?k—³îâÿÈ?Q€–éK>?PÏîôµ?j"Ú(U¸²?eh˜?[px?ï¬Íuê?tÍ<Õ^R?lq\¹f?PIº";?{Œd…Æ=?sö<€1?ïöœDÎ?Fi]c%¥œ>àBz;ˆÓþ>ÛP¿Èœ{?R§bSâù0?FVÝ="—OAGN3FGL J0019.1-5645@s{´?¢­?ÀMéE¿ý±qÀ:OÁä;~[À<mùÞý¿ä ìî¥{@;N	Î5@  €´ã¿ì;—"°BA¿Þ݊t¸Ž§¿ã'L]"H,¿ÑçeÈdeäAGNbcu?ïú©©Ý¯?=þ•Ò¸L[?.š(kQ
%?/NÀá¶þÏ?;e›\×Ýr?5"G§F<?ï¤2Ù_ñò?''mèÊP?a‰V8|ˆ?es&»p!?'ô	̺]?õÈ¢#_?îýu¥ãBÊ?‡H°s8?‰ò-ÜŸ{?~äýÓzoï?"X4S׉
?~©7#J?ï½^˜Øj?x¡gt%'F?%w!L'Ú?)•Ò‰—¹?€R}q¶ùÁ?xnã»6z?ïý{&£&?+ÊëúŠ¿Û?À~‹z_Ö?! ÿ÷a?*mUìîú€?"Þø+#½?ïâz•P?hgíiä?LQÃاýË?LÍ͆öO?fß^BØ?cQƒ×ñ?ý]ýü?ríé£*e§?u—'GJ?m˳÷ƒ¤¤?|eØþ¦?eùìï÷.?ïõ¶…¸',?Pòq™Åk?`éà}¿?èÞ<Þ<?SÏñRNh?Pª('_2AGN3FGL J0019.4+2021@\5ý~E€=ÀDð[ÿÛÀ:dZUÖÀ;ã]9–û¿áÕå
C@ñxô@ý1 6ç?ÚHtŸ|¿ë¢CgÄñr¿ÚESÔ	úL¿àû7Ê$Y"AGNbll?ïù}™¨?J€‡ÃðÅV?-ú؝Ý?é½]ðŸ?F(ð¿Jà¸?I¢Ç3Tâe?ïƒòtÀàõ?Ž*ÎÖTo?i´'A™#?|n	,€dà?ˆ–>TÖDe?…-è†ì·²?îƯ~H}?‹B␞íB?† T5	Ã?u;uâÞC±?›Ú
?=3?‡åÞ\:j>?ïIOBÇ%?ŽL†EÑ´?6ÁhøD
?:χ'¥!?–{,Õ;ª?ŽÈìâ?ïür«²åŠ?2&vߘ;?Ö£xÙ?9à¹lm?6µ?6ë?0'‡c¾‡#?ïØ=ÝõØÎ?nòx1}ó?RÂ2,?Qmkþ×½?nzœJX@?háú'm.Ž?ïuø$òÜ4?w:ù08ý?y>õ@®ÐÉ?d¹¥ûj*©?…â|+8Æ?t€vT¿x½?ïâú9}¶J?bÀ`hH?#ó­WUÃ&?ÙkŞÖ?kƋîÌÙ?b ƒÙ–ò9AGN3FGL J0021.6-6835@s01€
|[ÀH&a_–hÀ:J¾ò¶°À;ÿBûÅ¿â~Ž,öOŸ@–CPŒµ[@8B«v'¿äé©Cõg¿èÏÎ@F¿çú˜ž-8Y¿ïÿPÓP¹AGNbcu?ïèäÛêÕ?pÒ	#N?Nk5µŠOŽ?iHª$"b?_¬ùÌÍâ?`/ýÙÀ\?îÑ&G{? c`¸×–b?¹r^¸ŽO?ˆúý´6®?œþtèôÆr?˜ÈQ€X?íÌÖČ%W?•jo:å?¡Îœ´¾Ç?‰j"mÒ?¡c÷°­Ñ?Šì-ڏ?î—ÃM¦?µkü€Ù?‰ÇØÁÚ?†'drñ9>?¨%ÑÔQ.$?˜ê-·œ"ž?ï×»n3Aÿ?¦¥€K¢'R?pRÊ®µ?¦¦^¸—í?M±
è³
?H®£VÄ\ø?ïªÅä®É_?}m2â<X?gnZ'Gã?cÖÐ/|ª?~åà|Ô}J?w ïñ`q,?îه&¿ V?" Í$)6?–F‰m?{5Y³º?ˆ¿¶?Á?s›0X"ú?﨤ŒÅSd?xnÚÉ#?`€_<Ï´Ì?Vtb¬<?¶Äü_"º?vÙhè|û±AGN3FGL J0021.6-2553@Dçڟô&®ÀTÎ]?á—_À9¼º"eÀ;Ζ67Ê¿ûõõuã\@$|>M@ËVß_Ìn¿å<RÐÝS¿Þ®îñËðë¿ÜR¤J«'"¿ã>"¤âD{AGNbll?ïóü£ÌoÒ?WÝ0™d8?%—ø©¯!,?(¤ýT:R?US¹:FÁf?TöâVÃ!{?-jò<?–ÿ'*–I?b}[5ˆà}?{oÕ^Ќ?‰¾Ì2Œß?"®I­\¿Ö?ïPÚâJs¨?ö6¬¨'Æ?|'Ö­Ô¬?k»Åk—I?µ\H€®?~ƒñ§¦?ï«
jªKv?}e»"Œ¼?+Ír¡;Š? EuwÕ?…yxìï»?}QT¼[ï¢?ïúpâ^a?EŸ†"{›ž?I"ƒ'³?¶gÉEüñ?BóGãÒh?CìõŸÛ?ïÑNÓ͝?Œ&Ù@u&x?OÀ#í¿?RMõ~†i?s"Uá+'?‹Lʑ'Á?ï¶	x"~f?k{žƒ!«Ì?lE	ûӉÎ?X¾¤ø;Ë;?vؾÓ#ûË?gh':WÆ7?ïîҖ:iˆ?U†N•9½>çc>ë¿>ꞁߕ8€?a|Cæë?UzË[´4éAGN3FGL J0022.1-1855@Tû_ò®ßÀSØÊërªÀ98?±Æ·	À;NQ"GJA?ìˆÓY'Ž@ÞÊÏÇ~?üÈÇ>Ã_;?î¯ÎE.¨¿Ø.¬Ï¿ÐìBÅÿ坚ݼ^@AGNbll?ïî8,tÜ?Y+¦ÚœY˜?NDÀçÅþs?J¹/œ/âû?SÛ.ßs…?N&è§ì¿?îå«ÏëÔê? c瘐)?ƒ'ä<e£?•
=׸{?™‰ýrbò?"nÁ'ç|?e
ÿP? šâP	?'±pi¹Eö?"ù×–~ü?—:Âï_f?ˆs<Xbý?èñ¨þ€<ë?¶õ'C?•¡§	f(?'"I‡Ü£r?Ʌ:ߏ?µát¶3£Þ?ïõòöà¥$?HN"‰Ã1?Cþ^
7Ä?<šéFê?E1%
4Ç?;Gé6Œü?ïeÉ®	h4?"hi>럷?zâO…Ä8 ?ƒ³ÄqÃ>"?‰lÁKÀ?‰jãÀݔì?ïYÿؽÆÊ?"ŠÖý
(ä?ƒ"bÖcúP?t19ßxå?†]§y'?~{Ïý£?í-¤þ҃p?Ä!`*•³?•ì¿üò¿?\`:Á´£?±NØ"ÍR?›î¤Ò¡'ÏAGN3FGL J0022.1-5141@s™ìºËCÀP4߀-·ÉÀ9'컝oÀ;®,nóÓ¢?áDÂé–~@Vál)?ÿ̅>õ!?Ô.¢)àú¿ÙݪƐ¿æR¢¢Ša¡¿Ð0žú'¾ðAGNbll?ïæý¦º?a¤ó éG–?W|ú~n?U¬1´áÅ?ZˆÚÔRJK?Sρ'ÊÙ´?Gv?ŒœŒ,?f"F;(@*?g'ø¨Ú<•?ˆn©)OFÊ?ˆÓ†"¦ÞË?îwõéj?'Fޗ™r?™"g•ݺ?‰ÒcÒΟ?—ú9ªa6(?ƒ—¦¼â[?í˜Y¶ˆEg?¦¾$y˜-š?€"éù¥À;?›o5ƒ¡¶?±*µ­5Â?¥äò["3?ïõ·?
Ç?Që-&©?Bà'Ù9ú?BoJ«]æ?H¤ çÖ8?E#¦á\?ïØ(/@È?q‹Œ8¦›P?Rã¿ñ/Í4?Rs6?…y?neð'¬Aö?mL'ÿ wm?ïD7 cß?"ÃeSK?‹¸ü‡æÃã?œ†#"0ƒ?ƒBu áü{?pû&	P¢	?ï})•Œ?…ä
±'ãp?f?|jû?\ý|co?‹%øžHK?"4²¤)'íAGN3FGL J0022.5+0608@['¾‹ÁjÀL V·À8s¹NjÇÀ;:ÑY#‡Å?ì½Ã²œÊÑ@9aÜ>ò@–_¡PG¿Øÿçƒ~Ç~¿âœ§jŠò¿àjT7˜PL¿ãi,¶0BAGNbll?ïéßúüàç?~¹f¿*æq?+£#Ò)' ?8…yÔw`¥?deÒ¸a?g?}xjoÁv0?ï2úbˆ?"úD¨q:å?vƒ²YˆwR?zÉV…#¿?"ô.ö?'þé1t|?íï•N'͜?ž/¦:ë?'¾ãÕ??"×`K/®b?¨'9•M¿?šÔˆK÷ õ?êÂ×Ú?­Íw[p
?Ç=Ù,?"ötlâ¢?êÕQçºu?¬Þõ?X?ïé:ÎvÐ?²ºÔ‡K?@ôL'ÕÓO?|ðÿÜ?bˆgøF?–{u"K´?ï±ôœ?~ŒãžS?d»4ñÀØ?`Ûθ€?|¨þ\(­?y¸Ý鋂?ï32Sܘ?ŽÔ£h¡ëR?…xãÖ#™ª?¸QHÿ™š?''ÈºÒ ?Š^ýkš?î(¡gvåB?"ø"\æ ?‡`Áão
š?q—[¥¼îV?§¹'Ït?'­2oõùAGN3FGL J0023.4+0923@[Ý? §?ÀJmÎÿ¬óéÀ9¥:¿ïn¸À;×Ájî‹?ûðT5:Ÿ@ƒ`–mÀ"?øbÀú†™b?µ±¬lÒ]¨¿âç·¬ §7¿ìÒÈ'²²«¿ç…¨á$PSRPSR?ä+@ÿt?ÈÝÐGx?ÄØYcÚ¬?Á˜OË"l?Êz¦~V?Ça²Œ‡?årLü»……?΀%GjÖ@?Å}Ñò¦{)?ÄÁés:y?ĸúknÂ?À7øʁ˜ò?Üh}zݟa?·Ã"º/ÜÕ?Ôþ‹‰"‰?¶}HƧ~?Í1í÷Š-?²…ý/('5?Õ¢qg~òØ?ÁY‡Ê~Ò?ÞÀ7ç?Å)´"^ÛÇ?Ç;ô"'?¿åÖÛÞ'?êƒua<A5?Âx¤·/É?¼Ç— öù$?º›yåìzß?®9{«)áf?·–+ËSÞ¡?ë"Jhµž?Ãy{ñ+ë…?³ˆs!ºÙ¾?»»0"×Éç?°U9œ/«Q?°Ò'þ©g
?áFPB§^B?¸^‹ÿç§?ÑosÀÁü?³›+ œâ?È×sލÙ?°ü99(	?ã;b‡ÈQ?¹µÓ1Ñð^?Õf­P',6?¶Èéÿ'»½?°Š6‰BÎ ?¥Æxª"MIXED3FGL J0023.5+4454@]oâއ	tÀ1¯X?\6bÀ9 Q¯<ÜÀ;¼fÉbµ¿õ°¸´çÓ¹@ú@'7|n@ŒF JÎ/¿çôª}±J¿å´³5ˆ¿è¿`ÉLc¿å¿½Ù{4AGNfsrq?ïô°ê5?NbÖïWDt?<² øa?8.<èÑ:?Næ‹ÝgÓe?HË{<h¢þ?ïYÊ#"ó?"b<'|ƒ?sibiØ_?xN˜ô–?N5§ˆ™?Ï-事I?ï	Ík\?ƒzø€ní?"Ö©"P¯?p=ncH™^?"[0Èl7?~¡ž?NR?ïcbQ*ë?‰zEI÷?Hïò÷Bê?MLa]`#?'Ó®ZŸG~?‰ëàÊkÛ?ïùûSÝß?BŒí¶<?1©ý¥{l?)©;­!¿µ??!2ƒ¨Ä??'Tn…z?ïÍÒ'C ?s8E®ma?Y'X»®C?Tú9"ÞH?rÍF±öÎ?o̖`ôö?ïœHÆ9Ø?k…ļ'M?tÄ+µ-Ó\?bY©H÷T?}7¯Ê(œÈ?bö÷n?ï俺7b?a€2®æ?
'"AO?tPŠ¼c¯?jŒM"?…?aT9M¶œAGN3FGL J0023.9-7203@s©_ªŠƒÀFs¡€èTÀ8^½ÇvK·À;f-ù7Žã@¶@)æ®J@ø	24?ö"»J}¿µtDJ‡¸œ¿ÛÍ:°ÕöA¿æš*ž9;‹¿î#J]'OTHERglc?R XMMþ?Q¤ÍÊ
?ïÄœeHQ?ƒÐ7'à|?yi›çµ?'í¶é(?jL–ƒ%)?^ÒoåE^?ísF]ÿ²?º•lZ@?³''®§Õ?¹ŒøšÁÿ?•ØÙá¸`<?Š=)M£™D?í½"!8?œ6€v†9Ø?©:`úÆÏ?—Œ6Šh•?v'Æ}[U%?pʂõZ6
?î²TöŸ?˜«-¸~¿?¢ÅN©0e?—	p
RP?1ìÆÐ{?3²(ŠgÛ?ïãØV¶—?tbþD?iê'`k?sÎ"H¨e?y_¥ÿï°?Š9ÿ*BÝ?íl͐?·3ŠÁÆ{¨?³™Kc^?µf×"Ü»è?¡l@ªq"?"çc–ÿ?ítÞ½ÿÄ? Nixø5ó?¥Œqec€/?˜6h>O=w?Ž¼"$ͅS?z˜£7řž?îz¸ï[~<?'ߛ¤ææ? ¥Ký¥í?
ý¿iÿüPSR3FGL J0024.4+0350@[M–ÃüÀM,Úÿ•võÀ:Þ
ò}À;¾Êe€?ðAUÈ3‹@DpýC77@9ÎÀ—à1¿àëÝ3L]§¿æ¼,ÆÝt¿ç¼æç;t1¿åÀ|µ2AGNfsrq?ïÒ¤µŠ?€âӟþÑ??Y%\ßí¤}?`
BÃ|÷Œ?p«Ösnօ?~T$¥Û?ïI"õ·k€?˜i{,¢õ?ua¡öTnŽ?€Bu¤Q˜v?'vøÎÁJ?'²¯*ª—|?íß.À¸?B‡!Ž0?–Þ–Èô?‹ÇñƬLO?§¤ðW?™VSTØø¿?ì쩼Qz?¥¡ËU, ?•òˆ±"d?Ó'-BÒ?³ïéÜ?¢èï"z7Û?ïãIÑ«?ˆó…«ø'?LUñû8?ba<Ó®?e¡h²©ZŒ?"X)µL§Ê?ïÈDö?y,ͱõ?[Å$ýÝ[P?[ŒTßÅÁ?u
"jp
N?t•àœn?ïŸI©8À?^Ïã€è?†Ç•×øaì?€~lಖ˜?'¨KÞܶþ?Š3VùÉÌ?ïÉD4ÀÛ?‡Îìâ–ã‡?‰úÒ§T?xÙÎOEBî?›Kõý?€9ÄSúщAGN3FGL J0025.7+6404@^@¿ã°?õgq¡-ÒÀ9Ë/þËLšÀ;5í£ùo¿À¤®'À•@Œ-ëÉ@±§¶Cž?ëÿ&ò³¿çú
½'×á¿æ;×F£R¿Åoúä¸%÷OTHERsnr?î!ÌÇ»¸?§bÜÑÏ+|?ŠøSLþíN?ŒK•d1¬?§0n_h¢)?£Àe6R²?ÃQøp>¬?Ìc+!ۋÆ?°3'$h1p?®\%‹•?é6Ɲ€%w?ÍÁß;Ì?ë(9½ïlè?¨'d&žU?¨iœ?˜¡"ˆ?º¶$\ß1²?£ÆÀÌÁí©?èæ¼më&:?º]]¤ÜÿÜ?…œÚ«?Œa2g3Õ?ËL{ûñJ?ºO…ZTW?ï]öCfA?™(¨܆?un2Þ?°x³d?ô`'Dž[?"1x£ߌ?Òr)}§ËŒ?Õ²34q?±†]¡Î?¯üÓÞ`‰]?ä–(õ±aP?Ô{ 됏ã?î?L='ª?™q‹×Õ?˜WV)â?ˆöwH¿j?£¸ß5ý?"uRl¦5?íñ,°&?š·–sG"?p0µañ–—?fO²[æ'g?®çJ­s!?š-^DõKžMIXED3FGL J0026.7-4603@s½¿ "`ÀQœˆô'À:'–Æ€'qÀ<é¾u5¿ð¹1ø¶Õ@)v'hO @šK`%¯'¿â·4¶&Sb¿é'JO¯j¼¿Þú†¡øÁP¿è.4v)R	AGNbll?ï÷zÞ¢ß?Ng»Œ›ÌÕ?ŒþàÊûç?áÐ"Û9#?Oè,™¤ù?M=s*­¯?ïŸÛ¥á.6?"¥ž‡*†?b\¯"‹ú~?d.Þ¬G˜?ƒqê•jùß?€Î
ܺë?îtLÊÅ?'¥¾òÂËY?‰ònž£•?tPˆ@ôA|?¢:oŽ>'Ù?"]Šæª?ï‡Bgê± ?Î®Â'YÅ?3OØ~ò	?;K¨ú	(?"çJê—?}Žâ°Â?ïü\—…˜0?5HŒgS4©?ÄÕòºA?+ق´G?99J¨vðÕ?3ªUwgŠ?ïß»@ÕªŽ?ie¬ºÛ#?PDq%Bk?Q?ÆJ™Úœ?h"¾þÑTc?bÒdŸ
6?ïpj¾1Jó?|'|»N_ˆ?yd=
4‹?j6£Ú(¸?‡31éX´ý?xÓJô|µy?ïëęD­?U°ô´ZU°?\ˆáC?¦Â3{V«?c€'NªÚ?UE¶C¤"§AGN3FGL J0028.6+7507@^[òà\̊@( Q¿æ4}À9µ´v"±ÓÀ;™Ž"¬Ï¿ìº+­Wçs@
~kjÝ@»M DC&¿æG9H‡>‰¿ãÄ`óhu"¿Ü`†ÜX¿îÈ·ôoöTAGNbcu?ät¾—Äœ?Æƍ­ýÿ ?Î4*ÐÁ­?ÁÍF؊"â?¿ò
ì9›ú?¹íxÜé-3?ê­¾ªMÎ?Æj¬œ*Ãx?«NŸ¾Tlœ?±cêXuxW?¼êºÒ¾?ÁªE*#?èVÁ
h?¯wà×Þ³0?ÂêçpxIN?§áå…ýÆÅ?¹O{q—¢?ŸOБ—0x?ë'ÇÏEF?® Bêã—?›_DoVá?œ¾ÄÔäQ?¼'ðmeß?¨¦ ½Í?êž/›#2?¿ŸTŒ§Ì@?¾¬âæX}ß?¹€·~¬?¨ÄG=èT#?§¬NՊ'i?î«CÔÚÒ
?«•hïnŸ?Œ•ÒI?ba?"Ê´Jž)Ž?œLœFåE(?¤Òuá·?ìZ|*rð8?¡áp
}BÖ?²ì«*é¾?œ–׳µÃ?¤~çv÷	?‹g$æÚ¹?îæÄ%%?Ž?ñ}Hd¥?sI%‡º?lv9`Õs?žU2œ'A?‹ñg¯éF"AGN3FGL J0028.8+1951@\ë°À&ÌÀEYÝà‡kÀ9üaCöÈÀ;Ë«Ä>ˆÒ?åÉoïxð@šÀ`-@x+ßVè¿æ‹ƒˆ±¿à›º%'p¿î°-ʓŒ?¢MLu4ƗAGNbcu?í‹8+`?·ý"–ªš×?¡x"PÚc
?¦<yHgœ?¥ÓꎮÍì?²ŸûÖB?ïÈ,1¿É?ªíÑ
Ö?~ϼq&?—KÚÒ|—´?•³6ƒ˚? ¾^:—n?ì/sÛw"?£ïs¿æ?¦þèñÏ_?"h1L?a?³o說·? ¶A)œÚ·?ìú›o»,o?±âBy.Å?˜ý·\jg'?¥ñës¹²ª?±ë¶«¤?­yôTÿuf?ï)AìÕO?¬¦0¤å1…?†fÓåh?¦
n/a?H±Æi±?5îk±h"?ﰒ^çÁñ?"ímë»±d?j7·1$'?‡ù &‹æñ?zšôå$€?…I 	©¯¹?îŒ.[ ü¿?'ô7¯J¯?"!ÄÍ`,?'¾e"-<?›Y×?5"©£N?†E‡?‡¼™+"4X?qžóåYOk?t¯†'F?†AEŸ»T|?'Bà¹4‡ÑAGN3FGL J0029.1-7045@sKÀ]RÁÀG!?©c;À9Žslf×À;ÂDw(UŠ¿ß:]¦Ã@>-_‰¨`@F±_ˆü"¿èm:$¶e$¿áBf=1ö¿à!Ô³mx¿çbN°«ó¨AGNbll?ïñøP&o?SfP)U¿E?D<'"­ ¶?CñŽõß?QñÕøN±?Lª|Mv(?ï]¬"œTŠ?'"^,?p¡8w}S€?€…*…'a#?"iÆ¥é?ˆÅ¶nk·l?ï-M}%4?'¸ƒ"y_ß?'Ú0.dK?nó²·T?ï~<@Ú?}­|3õ?ï!µÖ?‹ˆ|ÐÏ?Z~´YêÔ?SÐ*~?š5;ÖWÖz?Š¼´F†0¸?ïúŽ‹|Õ?=•-ąþ[?1ðŒg>Ý`?-áëÉ­?9›'ð"—?4u£Š'?ïÑkD>Û?qQ*€¹NB?VÛw¦§ä~?TGYtP?q"€
‰iH?k³Ëdèðî?輸ÊA¤ˆ?j"à(ç]?qOÈýû¼ü?`Ð#JB?xîÑÛ²ŸK?a÷éª?ïÓPÔ¦,q?gYwûš+Ä?=¶˜ƒzîB?4¥¦j[Î?t|,!Ï95?fÅ4 œÄNAGN3FGL J0030.2-1646@X!T€uÀS¢î «†À:ÆÌ؋GÀ;Ôač?Òd
VæÓ@§rëZ§?úZê:GÏ¿ïœ Rc'º?ïÿ™¤ðÿv¿×mÓôv¿Úbêc",¦AGNbcu?ïþ¹©ç?)ÀpM¢‰5?/Ì.ûë/?~òkµ?)yÔ´¾x?'ï!AÒ?Àüt?‰É$Öáê?iÚ¶ñ"ª?p
ᒊ?ˆå0C
%?…BIh¹-Ý?ïYÃÿ8?¢§Ü¾·? x܎Ïz?w=ÒjØƒ?—,½îВ0?Û¡	Vi?ï	(ý>Œ?™‡Æ<ÖC?sÜKÿŠŸ¹?q–Ï3EL?™ãÍ_èʏ?˜tpøã•?ïþ—†ÞšÄ? rĀM(ø?$"O…>úNË®À³?!þjZI°³?"gŠ7ä–?ïÙAG_»?mewvˆ²?S¡˜#td±?Qþj:7•?lîàŸ'\?fôç[¸õ??ïjñ	º`[?‹­é¹•Ù?rØ葴ÕÙ?qnÉhìŒ?‹×IH5ˆT?‰fÕ¯Æíë?ﵞÜ4Úä?wµÌéDØ?_Ö5Ûöâ¨?Q—{C"šr?};†¢?uùЍŒöAGN3FGL J0030.3-4223@sÔÖàL'ÀRˆð€0<À8¥§
›duÀ;¼^¸; ?ÚJ"Õߒo@‰«Ó
@¤ë€—.¿åÚÎÙ¨Ž¿æÒhõk¿é•";
ºf¿çí)]5TAGNfsrq?ï÷$ظ¤ˆ?S".rè)?EöñþiÔ&?NyšÅ'°ì?:ëVqµk?D³Ð?ÖÏd?ïvòÝzŠ?"°üfâE?nY[Üñõ?zhk?Š¬ñ϶m,?\ð8:BÂ?íÝ;¥ƒÄ?œ³¶U…ü*?'—zºÄ'?ˆ)žÇÇM‰?©, ‰&H®?š…Ñgp{?ï"nm¿?šGåí'/Á?o'‡¬Ó!l?n¥}uE*B?›iC¤?™W֗+,?ïú9Ü3‹â?K½à/\?=‡¹½éj?E"$r0Â?1–iý]?7æ¥eb;?ïÔ^Ç5´?r¿¡r¥?V5Ži$0?U1*Îr?pOOQ?l¢ä"Q7?î½³ÞÙª?–à7ýa.?ïß)°M?Œ0*©Ç›'?˜Q½5JҜ?×…Üz<?ïÖÀ^²ñb?t	òI—y]?H©BÐ
Í?=×kÎ[Ú?qŠ¨WP¥?sD'ðAGN3FGL J0030.4+0451@\Ie¶™…ÀL͵_ȽtÀ7††*QbÀ;8k)«@­ï`J˜€@:֑ó?ÿ,-Z+¿Á7#§=àпÞ°NxR¿çîßNã¿î&Çy­¦PSRPSR?c-ó"üù?e)"èù»?ïä-†Bq6?kl†5íÚ?QI
­@)6?Q¾JVÑû
?€I_'€[ˆ?«ÚñLºÁþ?ìëã©eÈ?ÀÝxk¡?¶—¶ÀÞç]?¼"CñòK? xŸz¹lŽ?•ñËê½?ìs$£´‹Ê?§šguµ,Ö?´*‹$÷í?£GJµ?fR"kS@?h™Tã!Æü?ï,No¤¨–?'J¨W½û?—«ß•œ÷×?-s{ƒÌ+?XÍ°âÿž?d]_æZÓ?ïŬ–>–?§nIüѶç?vöocµ9?§b@•[]?‰†íÿÔ4k?®ŠF ÌN?여ݡ¹×?¾D«ý/§I?¸»R‰·:?¹rö½Û ?©'Þfâ"? .Î}.²y?ìPÖág}W?§BßGÓ?°°Y¿šýJ? S #í9?vôӗèL¯?gE̼Ö?ïAfY•?†¤',S>B?'!>T~¦\?"è¿¥ÕPSR3FGL J0030.7-0209@[¶ýŸÓo~ÀP"Ñ¿æ4}À95eWr­À;­7Ÿ©~?òJß³õ:@qa²øe@V_]2¶¿âo58WE¿åÍKaA'V¿æI×é2¿ïÿÒXÛlAGNbcu?ïâÛÐÜã?hÒÓ0_ü?RŸ2k<X?R µÎ »?cÔ¯äá?drž² Ù?ïƒ*ô¬…?ŒôÍf»?i†¦`Ø?t=5©žŒ?ˆÓ™3‡Û?†Br&²?íCcp×r?ŸV"öÂu£?¨hZ‹¤ª?—"?üUŒ¶?GzÕîj?ŽIÄ‹Ž?嗀™ÊÛ ?ƒ[ãà?\Ñ(ª*ÏÏ?aWfÜF?'BtfÕ²/?Â·)q?ïð9§§µw?`]ãW3E?HãznŸ0?LTŸšÆA?S†¾ÞÀ×?Xч†A"!?ïÖÊ>??qÆ].EÄ?UVÑ|ð¥Ÿ?T§Q"¤q?nŠ}×M,¤?kŠeÂÒ ?FÅY?ŒïðúŽ?œw!#Û	M?…óèÎЛ?Žh·\IÃH?}ye—'Œ?ïëö&ãD?c«Q'6,?Iìé #ª!?D?ø%†›g?\ãŸr±®O?ak•×m'µAGN3FGL J0031.3+0724@\ŒÿyÈCÀKŽÃ€ðÒÀ: &yÀ;Øöfú
?­òw7aC¦@ù䥆ŒÍ?ý.µÀ@ÍP¿îǨ )z?ëêDE:'ï¿èS´t³¨†?È®?-'_iAGNbcu?ïßšÜ?gfõÖjg?P@‡XoÒ?S÷""ÓÙr?h`"<Þ]9?dM1­_Å?ï‰W'%E¤?MC½Šˆ±?g:j® n?x¸‰WWÙÉ?‡Û-c?‹"É¢ƒŸž?îA*0z2?Rþ[äM?'ýoQÓy"?ìÜ4eaª?¢n¥X¢U?‰vq…´?ï´j«D'?›=àE?€æäÇ[œ?y±l«G?• ÿ/É?–«š
Œú?ïðÊ5äÎ?U3þs­­?;¡IsMXS?;)"¥?WƒC•xÇ?R{ôbÕò—?ï×8¾þŠ?wÏ(^YW?T*…·Ôàõ?b,¨$F?n±þäý¾-?pD¼q"­q?ï$Ç??W8?‡ºÐ%:ÚÄ?táŸ~ø8ú?@Œ"£q?xnp%úáî?ïØ=W4«j?qI£çk(¬?P|K´Þ"?R³r`€*€?o¸jv⦦?oT‰|ètMAGN3FGL J0032.3-2852@"Œ¼ÀO(ÀU\>ÏuÀ:®1ËT&ÉÀ<âP3ÀÌUàÝ%
@
²gEß]@"! 
Ñû¿Ö{ãaÈ¿æ
8$1Ë¿á¤û|§_¿Ù'ÈÇQLAGNbll?ïÔÒÁ>µY?oÇàù…_¡?NV"<fæ?UEp†R¥v?qËÛ
R>f?k¤Gl®¢?í\¾Õ=^°?Êä¦Iø"ò?eTENÙò?q¸-ót&§?´og,d+?ÊÀ뉾
?íÿC[cB?šçØ#¿Ž%?šXf^?Š"úcãô?¨óØÆ©gÛ?–'MiîšÎ?ï×â˜C¶Â?|i&d	Á'>Â[~"ñ·>ãÕCF?thfñN«?|gXóAñ´?ïñP_ól?T«4öâ_?/øpPŠ?1ŒQ7f A?Y{Ó`Þj?RôR53–?ï
ïzÕ;å?»J%Ÿï™?V·­Üì²u?g"Å6´QÁ?6•È'š@?ºñzZ}éª?ïr•ôžx?Œ}½Q!M?†ø¸4¥©;?wusÞ×3?"õQ(Ñ*a?ŠBñ?"?ïúªIÙב?G"ÿB¬—>y«Nr›<H>Ÿ0$ Ë~"?EV̞k>?G""¦]/ËAGN3FGL J0033.6-1921@W'¿ö$µÀTNW_ÍÅñÀ84©Tø€À:¯8hýœ?æócm_Á@¬¡fítã?ûo yÒ¿Þ¢þIh÷¿ÔÖhW¿Óëm"ΠڿÖù`ïYÂAGNbll?ïÆ×t'?"Üà'½·z?G¶Ñþ¨Þ?I%Þî?y˜v??"¤(:rð?ï>°$™ù?ž|c˜ò?x­¨´Z‹J?ö>%Νg?'þ'MÂA?•"/mÒ?ë"ÌŽÅD?²:Á£Íç?¤"ô‹R?š¨­d¥çž?¼Ü
†°w›?­²± }b?äœ'ú˜?»ŸLÔî?~€4É\?}Ý±—)a?×T"Û¶8{?»¦Âp°ö?ïç€#?¹î?o#‹æ½ó?@£añ…?@Jú®i*Ø?dW–¤…?mÝ*Âf6?XÉ|?•
À‰ƒ³?eÀ5ã-`²?t´ŽLgl`?ƒì\ƒ'\ì?'¸ôE=[?îÇý|j?¡zDõÀpz?•ÜÂÛ~¸º?'†u_±®?¤Å·ãø?›BY1n?éeNûTŽf?¯2&àî­?…{RüÜ?tÅ!R 6i?ɬaê£?¯@š¤ÜmÕAGN3FGL J0034.3-0534@[ß.ßç[ÄÀQº¿ïn¸À8½bð À;›ìVuX?þÍæ°M»@æ`pX,½@%G—ÙW'휿ٿáÕ`•Ó!·¿æA†û‡Jb¿î¨ö4­ºPSRPSR?}¡¡ä¸o&?xøØM?ï¯ñô"T?3øÎá×?dÊǪ:ª?i›Þ÷~r"?°#7 QÚî?ÀƒŸ¿£?è|ҶƦ?ÌÄè"¤ÖË?ÅûU*m¬?ÃþçJÁ3*?¾ÿ8@H?§#§`<çÎ?éÝ­bNSË?«§¿ÊvTr?²\®¸¬Þ?œí"µ²"‹?®[{FŠbv? û=%3òõ?ë"¡z0<?®æEµ:
È?·½6Œñúá?¦ðٖe°Õ?x^öžïý#?wWÆá‰pú?ï»8%høÆ?~)I:‰¦?d	페'?cJ—ôã ?º?¤ä.ù?ËÖÅ,»Ë?è"1ýö\à?Ð'~&ÃÜ?À"e–?¼XŽ£O·?ɅéG›ŽÖ?®ô|µ®?çÒsâñZ?±'Ò˜K?¬Á*'ªá
?›ÂÀâçI?Ä¢'~±Ñ?¨Û
C¤V?èüæÀ"Ù?«ñ4£/K?¯Ã§RG~!?œÄ"TPSR3FGL J0035.2+1513@]IP?³t6ÀG»ÒàD²À9OíhMÇÀ;P"Ý?à|[jVWr@¸e{.õa?üç€bæÕ¿ãÓ5»4P¿Ä¯Wíó¯¿ÚCRóà¿ÖEˆ–£+OAGNbll?ïçÚÑ¢®?^ú@JX¬?K—ÿ±,?H¦–pkž?a?.ýŽ£?W¿Äƒš?ïF8¥|ÀŠ?"·jâbeo?p"€](<?pº°QPò?"$±,‹¹?'+àCp?îФð\@j?‰×æ4æ?JŠàÅÝ?}öDZñêÉ?–FY«—óÒ?Ì×®…Â?ìGºg"+­?¤Ïf²¡o?ÊŠ3mü?}A/u8'A?»ˆÛ}·`?¤"¶X)'e?ïõºî9?M?H,uœؕ?;§ÔVZ£S?7_£·?K@]³Œ?@%Ó Mð?ïȱÆÐÎ(?va±¶¬?ZH$ý}~7?T­vô?ua(ˆc?rü›
6p<?ï縿?pí©mw~É?}P×±'?g>lIAÎë?´Ìœ4Û?bÚ|Gšè?®?…•1øBì?wkúxüF?b¥)žÏu?¡þÿ…ùØ?"v'š!õ`AGN3FGL J0035.9+5949@^?ßÖkÀÙß`£-íÀ83J‰'
ÚÀ:õWÁ‡õ,¿ÌçSÐ{qÕ@÷Õ±Lé"?þ]I^î¢à¿Ó}•?uil¿äÔîuOH¤¿Õò™ûiBd¿×á&$AGNbll?ïciŽäß¾?ŽÓ4V/ß?G(ÛÜLyP?FÝ{µ`>†?'Ù‡<—?Žb~21–Ö?æ!,}vx?Ð~öPåÜÏ? ¬6bÀÿ? ™'žäÃJ?Ѩ'Z¦®o?Ïó&öx?ëˆßàOáj?«¶·ðC_Ö?—Ý"0úêZ?Š³pBMÑq?½ÁŸòú?©jÿ¦7þ?ì?eÊÎߐ?¥´´}»\?Y(
°Ú¸O?V'`H8?½ 1t}f™?¥¯ÍÌFØ?ïÌ(^\Æn?qý?DZ@?Cíóù?@µ
f>#N?w~—;ñŸÌ?p'ɱr?ìy9¿`Êè?ÃMµT=Í?Næ8×?'?«êé"8?¸"¯٘†?Á£=-M:?îŒÊ	5¼?˜)¥Tˆ¤?‰#¤<:?÷ˆÙt"V? ê—5»-?"ûíoÜ;=?îÖ#"Íh?"ÿx©[™ß?N!Á7ÓÞ?>ÖØ{Ÿj?¢%FÑï£?"ØXäK-KAGN3FGL J0037.9+1239@]r7`¿]yÀI
Ô¿àU@À9PäEVÀ;ŠG?¿ÕKÐõ%†@Èé¬+—ˆ@6<6[²¿â	ÚIb¿å¶ì"çʙ¿ÝÂÈïiý¿ã&ã
?¸ÁAGNbll?ïñÝc¯
/?SÃ5\ø»R?!úOz"ó?çC–[?Zös>-?SÔ?
Û+?ïp3ˆ‡gW?99Œ²Ž/?j><®f?hȚc(@?cšR†Ê?Šbi˃s(?ï2<l†ªÃ?"+ØSDFë?Zð¥eÈæ?iIñì_?'á¶H8ïY?"Š–®B?îr÷ZƒÈç?'ÊŸõÈ?UZ֏í?P:í`¿c?¨%³¦‡ª?'¢Â3×øï?ïúˆË|Pð?@,h(f8?G۔×÷¸?¦Œ;Y9C?AóÖ#»À?<¬[ÎqÂ4?ïÔÉ`[µ]?p·ØÆk?SúXÞ¬à×?RœêŸW1?pœ¹"šá?kbõÏï¦Ê?ﰂ¬ö¡:?j"ßž×3=?nE	E¸>Ë?Yÿï‰o:Ú?xœ$è²{|?eˆÿfÎ?ï¤Tœÿ"?p
LR¬b?C/DžE'Ç?2÷¢"ï¯?…·ÜHíd?o¶I(ÄžAGN3FGL J0038.0-2501@PÂê /JpÀU•IÿþRÀ9ÀF¯ç¹¸À;á"Év7?ãLL@µ>@«õ–?G@'ã@V²>¿åkñ&!U¿å|CåÝê׿ç¤NyhT¿ìÁ‡§Ý2AGNfsrq?ïòÓ\3¾?Tt}z£Ç?L¨tÅ*õ?KÔv[!Ù?H±åЇÌý?G•™ê£uÔ?îÕ®ñx0q?§Ô!©?uÁ³ì¼Ž_?z;ŠŽ	?ŸÙ´Û¢$C?¥çEîӆ?î5Züꐜ?¡àéè¦?ŒVâÑ 7'?yóBêÏ®â?¥"—z{3b?¡xýŽRì÷?îƒ9«ûÏw?˜Ç;Itl?'ð+½Æ9?x›¼Þ¿?£Di3ÇÃÿ?–xiÊÔ7?ïôCض©º?{­ =Æâ¸?C'ã<6¯?@ˆõÿkp"?K^¹ÿê~?{…ÆÊE†7?ï‹oÛÒµ?'ããzõOß?eúžú¤E?iŒâ^~ð\?‡¥®³#‡?'hèá	Ù?î¿h,(ã?:si:H?…ÁÚ°"$?{•þêä2m?2
"Ço?œþì^¬k?אַgî?uå
Ñ(Gæ?j ­«?VÚ¼u§?|˜Ã©54•?s[C¼#!AGN3FGL J0038.0+0012@\ì  ô×®ÀO<¾Ÿã_¶À:[¯ˆïÀ;Õ
»ªeš¿×:]ã¤Ä@'QS"·@@›àEÐo¿Ör:ˆD»$¿æì•^ÃÒ¿Õ"˜Ue§¿åXNRÉP–AGNbll?ïÒinÙ|‰?zví÷,°W?;ᚐÖ^?8˜õ¤û?u
8h¢cì?yÙ+b^?îþs²÷†?£V¨ÞO?~ø¤ÓÔ#?‰ìKì]Mó?˜s`n˜ê?1ÝP[?Ê?îR^ˆ»>Ê?Ž,§q×/h?'ùðïhP?}Ø8"̬Ã?¡ÝjÔ_=?†<+<p?ìE Eš¿?¦þ.ŸžÃ?|ãØ\A?weÛÙ?½lx½ðª¼?¦¾ƒ1C?ïë™HÞ?'²?ߒAú?-Œ%Ãê§Å?7p.wÿ¡+?be6ÔÊ?'€ŠJº?ïÂ0Y?y&}J¿?aÔ~Saa?`!Y_ûdÑ?vY7›.?s;(W/V?ïP.¥ž¤_?w	½yÕ?'ÍÒ¥6­?l+0¸"?ŠaˆÇiƒ?p§er-U?ï
"q]Õ?‡+cv–$?iŽùŒ"As?Wà"§©ƒ›?›Œ\…—")?†!჋ÖAGN3FGL J0039.0-2218@VúQ?ùSÀUp¿ñ7À:ÊËi~KÀ;çåPQQ+?ï¡¿#R%Î@Ë+1¥?ûr"^úŒN?îÚ²ämà¿ág5离¿Ë3^ÿ6Mç¿àÆ<¥ÖF|AGNbcu?ïÐ5s:›n?qʀfÌ£–?O©MѼ?Hļ?sð&'n"k?p¶'Í1ø?îÏù>½!€?¦6\Åi0d?†K¤:©Á?—oº÷7ô?šø2O_C?›‰5`á?ìê-ÝL»‰?¢
ž©ù¹?¥¾ê!?•¦¯X}¤?«Ìc@M?Q?—‰nÎ+þ?êwHæ±?´s5o¸˜?—§Ë<})Ž?œÁ?Ã÷Ÿ?Ã-âþß»ß?²GÿܺBÁ?ïÛ
c¯– ?hï‡RÀOe?NFŽ{½è?F9)'al‹?m`øÒßíX?eÎââ	i?á[$>?Ùòjÿ:?o›ª±À#?F5õ'…?€·]5H¥?'²3Ž`Í?îÔ'ؤ
?"]EjN~?–¯Qõg¶ù?ˆ
i~¬?—6ª\]Å?ˆ㚃IW?îe‡ÌÆ?@ˆ[XÁ7?šÅ+)	Ë?'âwiÀy?¢qÄëd(?"ƒcgÒyAGN3FGL J0039.1-0939@\:'@·€4ÀRŠ4fÀ:E$oKvÀ;ß¹Z)AB?í"Ìû=@´¶|ï@ÀsÀ—	q¿ÚR)³W°Á¿êº"vØà"¿í›RÙw¿ïý_"î—«AGNfsrq?î\À¯Õg?¬ù9.£@1?"ÙÔ7ÉG?" 	l²¨+?¢Î¾‹ãÅÚ?©)I›«Å?é¦ë'=bj?ÂùZðøŒT?·ÙÚ吊?¸"Y'‹Å?ºîÉP/\(?´ˆ±4­ì?é[âj	?¯Fï áVZ?¼$t¥)«Ü?£v'Û98?¸üx&-Ý?¢½]ì_Þ9?á~ÆÓtÂÜ?¹1 ý`?Ñyϳ¾´?¸£Õ	hO?ÇFªÅw)?´ÎÀÐ?î‰T®iE¥?¬"@¤ŠäJ?Š°ŒUWX?Œñ†tá™Ý? ¾²4žÜ?¨-ò›WM´?íQGG3p?³‰Á¹Ç?¦XÝX3"m?©=ÊéWMî?¤'®8¥‹? ìæ÷à¹?ìµB‡dð? å‹öÈèŸ?¯4÷ž%¨-?–ÃÉÕé9?¥vßè)ìÛ?'#]yÄd?êY«©4[?§ÿ¡ž;c?¿s¹,©M¹?¡š_–'QÃ?«}Ü¢oÔ?šÂ÷dd©YAGN3FGL J0039.1+4330@^%~0‡‡À3PlÀ»"À:Mq
"À;àÎs•ùÒ?㽝lb@Šz¥7²t?ÿgîÿQ¯J¿éD ±³8¿Á'cÿj¿áÔ?®#ȿݘҔŒê_AGNbcu?ïçÊAW8K?_dcˆsÐ?GۄPDê?D§°hÞݙ?b>Ý«UO†?Z5"ý«?íßü,5èð?³}îµñ7<?•¹PSÏ?–°iJäƒ6?§w`¬å'?°o|è…{Z?î'0ûå-?ŒÉ½E³M?D™sûÜ?gQH¡?ŸuFùś"?"h¸ߞ?ìRlD²ô?§'oó=Ü?§"c±o ?¡ÎøÞéþã?¯èu‹!¥¥?]þÄÞÅ1?ïöÇ|ÖÀA?F]•¬ýƒ?0'µ6q˜×?)Ð8çÉ9Õ?L˜²ŸNÉÕ?C4/¡X¾c?ïWË¢œÁ?œö {}R?z¼›?•N?ýdyç ?Œ¯¬Ù,ü?—0& k©s?ïa@K}5?s¦Z¼ž?2è‹'e?g£¼†y?ˆ ¦sÉ1?j=êޑ	?îòäV+ZÍ?‡­\iïO1?"fœeS?"egYFÀ?‹
Ù§ð'0?v¡"£_dðAGN3FGL J0040.3+4049@^*§"X¼À6J_Ÿ¢ÈÀ:³t«£‡YÀ;³6nQs?ÔuüÎ-†@HG§‰qX?òºÀۧܿç@ÈôfL¿èXBd‡Æ¿Ùîh§Íþ•?Ôð3ásAGNbcu?ï]oZ3…Ç?œöGr›?"YTUst?#Äz§;ÇÅ?"-b~$Q?œðÑ{í"?ïvg•\ë?.CN?p1_é]Þ?vQàŒŽ?Šeö+ÂO?ˆ&5µÍ~?í èékœ?ž`&…}×?œð´2¢¼?"Ý<¿J™†?§yT@°0?˜?šÍ?îŠbQƒÖ9?ª®jPÊ«‡?Q6dŽr–?nWi¢Ë¼j?¦Ð'ÀÑPq?ª´)݆ôÊ?ïsZ›Z?"îð–´£?%$…"U¤(?*J¯f*›?ˆN—lâ(?"á
j"Â?ïϚªeÄ«?rÖDÀ-gü?YÜ×Èâ™?[>`zÌt?q»u%Ù¹?kôÚ¼0hÅ?ìç"
'?¨zìê«X?«#TU@?¡Ã[l´Ê}?¦c{}êß?L".¸?ïÁwÓc·?z¡ç;¦??ýœu6?PL·J4‹B?}S†½"g|?y–	0ºAGN3FGL J0040.5-2339@UÊá`ÈWÀUoÌþ£	À:ߍ'ûÀ<ϗ'h%?Ô½
˜Æq$@,҃Åò¾?ÿ#¹€iÇÅ?ïŒp3:a¿äX­šúº¿ä77	¯¨¿¦"ãæ*',AGNbcu?ïø¬k®é?D"ªÌ£žÒ?%¼k>¢v?%¤¾¹ó‰?Hãþæ?Aw|Yؽ?­Ý7B?'¨VƗEÛ?b»l©ï¦?fÜÁäÚ?†®y`Ð5ž?'Y³"ø?§?î‹ùÁU(?•r'aY;z?Œ>¿°
$?|5üu`Ç? 0³ú^yŠ?"ïTdšÚ?ï>ï:F3?™È :"?MВ©	T?YЛÍí.?ž«"yçP?˜ÁJ>Õ?ïûíڂÔ?5"½Ÿ.? Z1iÙ9)?$™i¸w?8j3¤?0bßçò?ïߍíûù?mŸÁAÏ?M—}û;å?P:š"Ö9ð?i2V¸?gü›qâý°?ïJíõ™þ!?‰"JOY"?€Ð`–,?uðµñ§??Œtk8'€'?‡ÄÔÊÕÎ?ïÜ\‰¾$?pT`ôœR'?;jë¦Þ[?Aȅƒòêl?pÕOF?o3⣀OªAGN3FGL J0041.9+3639@^4´A»Œ3À:+ä€G¸üÀ:»•EwÀ;÷ÇúÕô"ÀñçßÃ@bg¦'`B?ÿœ»úl?ïþÁVw¿î7à†4¿Å#»L'ö¦?¤»ùë¾ÕhAGNbll?ᅣÂÇæ3?‰[Œxç?ÄAä8z?!{ß4˜?ƍyïêè?‰Ouóœü?ïýv?'—Â"%¤?iõ-Õ­qj?|xÌVǘI?…¼5Oíþ÷?>©9óâR?í"ÊÅ`œÎ?¡]髄ò{?‰."%?x¦"ýœ.:?°·¦Nº¡r?¡5×Êe
?ï²ÞnWBÿ?'«àSGfÐ>àùµŽÉ–>ü¿›õ?ƒD%ïáÎ^?'©¥ÄË?ïÝÏðSö³?zD‹Nk§?X|ûc˜?äîՅâ/?p®¥ÀÔ|?z.Œ·‰EÆ?ï×¾–0áþ?rRŒù"ð3?TÔWÓú=?S ޘ	uA?m×>"ù÷Í?p4kA?î~¨—c^t?™…H…©~?'xø2*óg?#	S=¥4?£w8{߃å?˜—âu·?ïöЖ?Naø †£X>½+L±k>ÄnwÐs?SÀþ©èíý?N[.-XCAGN3FGL J0042.0+2318@^	F^‰"SÀCÂߥ¥À:‹ ²'À;Ð:‰hÊ?ØÄ·omv%@¥¥À‰d@Õݟ­ÚÄ¿âxj
K(Y¿ç<4–,8¿àn–
ÃÓ¿ïÿÄ^œÌAGNfsrq?ïű8'äˆ?|-"'"1?K2Èq0pÿ?F NR¦® ?yÁ
™Ýqk?{q–IÈÁ?ìðÀtR8?¬ý‡¸m0? š§ÆäóŽ?œ¯êâä¯?°,¨}jÂt?¤ú騖?ìå½ëÍ1æ? ÕVo-¤?§åt*͝¨?"rõ2JÅ?©¾­_Cô?—=Š}†Ž[?ëïÿÅ{'q?§·"óðè?¤ÍŠCݜË?š¬;—6¼?¶<²7ö? ²"u¢xÎ?ïìaPŽ"?`ùŸ–X?<5OÏ?4"Úᪿj?`¬Cb{Û?]ç_ü+?î˯•H?ú?—í3ë,è?è5c-.´?ˆÆZ]g»Û?–•òž'1?*?3½4?îWç.?E!È&ÊÅ?™¸Z.™X?§Íæ'?"eÃ0õHõ?"^Ѧ44v?îºT5ûÿ.?ˆ'`ìÓ6?"S€Ø	«?|Qyæ:"?"aøaˆØ˜?€½»ØuÜØAGN3FGL J0042.5+4117@^He¶™…À5‹x_.QÀ9ÛÌ`–BÍÀ;Ç6oþ•?ãˆ=ZmM¥@
kzÜÀ
@¥ŸŒLտṙaܔ¿âÛ
½Wäÿí7ž­)Ä¿âæa(9.OTHERgal?·²?¢¯…eåJ?r¶'	´? !´Ðiªã?‰5å ?Šªó8eYó?ìÉ:±Â¸?ĕ¯Û‹'¬?¤…
Þtpé?³	GÅo?®çG"|"?¾Z">C+?ì"cNjÖ?¢ìL˜ž?§hCnµW?•ÈÖò5T?¯gAƒˆ)=?—Õ»åö?ægŒ¬/?»°¼¬Ÿ ?Æ=nB?¼CXß?À$¸Aáˆ?°1á"#ß?ï»fyx?'£UÒ¾Ø?p±nc<;?vL#üªÒ#?rH@èP×v?v37݋e?îɿ؃Ëb?±Héˆ,Ob?Š°eùRg?—˸O߉?™oÒ!ª²Œ?©ÙàzŒ`?îØ\&`UÅ?ˆØÙÑÈ?'î¼w[?¡z×ø%?'âŒuÆ`	?yE¸™€™i?íaåML9?è2}¯N?¦åt¾ŒÐÛ?"½Ÿ´ðõç? $lê杖?'üq(ìcAGN3FGL J0043.5-0444@]rö@c^ÀPâŸÞW9À:‰¤f|5ÜÀ;Èà¨KäÀ
ÉlüX@
'¹Özök?ûÀÝ "šY¿ì5aËÞ!¿Òƒw³¼½¿Ð´
¤¿x¸¿Æ±
3oC/AGNbcu?ïón³Ö z?U>tøUÝ?#	êoÀÏ?îUêU´Œ?VÁ[T7ƒ[?T-'ZA1?ï­½j%°
?‰OŒ>Ä	O?aúíl¸ŽŸ?|6íU
?ې
OsÜ?G4/§}?îßKZyü¤?†€‡àð¬a?"óVÝ2?n¡$H?™œé9§Ü÷?ƒPEÅí?ïêcžÏ†?gK«MkÛ«>›×Üxý">±™›ôªV?eœ	œEa?gKŸ NL'?ïøí‡Ww¶?AêR‡‡;?따hŽ&?cbjá5?I,páý
¿?A%@'/«?ïä
IÁ%`?i-äîÝ?Iusïpñ?KÏêY"·®?e˜Y_c. ?dL¥sb:l?ï{®_ùH?r`ì	Ìü?y=b™wÀ?d°ÎÎáxK?"ŽÉ|£N*?iÃt EÀ3?ïüL®HA&?7ôi¥>iÿ$'á˜'>|Í[ƒÒ*þ?=™¾"®ö?7ó~HόyAGN3FGL J0043.7-1117@]žYò»ÀRƒ¢ÿßHÐÀ:O".bêÀ;r²¥Z?ç÷ lÿT+@
Aï8²?ùæÀ
¿ïþÏA­Z¨?ïú˜G£Ç¿Ò±á3·¥¿×‰ùÉ/3tAGNbcu?ïò9³ªçË?VÄìx¢ŸÆ?6²è¸B?9Ï &?V
´du?TË>Ô
u??î§ì1…Î?²Aèð©QÇ?•RRõÉú? TU¯±?¤X7€s#?¦Ùqðº'?î'KTš¿'?ŒUèËÎ"¢?ìÍ+?Ðk"Á?Ÿ¯¨–åô·?†)é'U¸?çí2Qû?ÁTiDoÏ?¼RÄTû|Z?´ó¶¸NÀ¡?Â"q:S—?¾ZºiP"0?ï÷†û?HcÓɌ¡?(ˆ£ýÈÌ?"rˆ@7›?KÂ%RWÊ?F8ۛ²¸0?ïxhëN?"þ"³P?xãµ<?"ú Öµêï?…t$¿ýÜd?Šaƒ5{£??ïHHsŒ>½?CÖ~ZX¦?'ª–1©G?tþJÆTð?‹CLõ•Ý'?y)ËpûAŠ?ëú5Õ=Î?¬}ÀÊ/ð{?°¡=ÃÁ¥?¡>i!ûª?¯ÑÒÏ?¤Â‹Ý¼AGN3FGL J0043.8+3425@^J:>À/0À<j'_8t¼À8¾Ž'b™À;Xó"
3¿íÓ>Bä_@žŽ5	L@[ŠI{õ¿Û¬š%8Q^¿ãʽ ßÞø¿ÚxÈՂ¿ã%NŽáã=AGNfsrq?ïý'cB3?*¯…¾Iã?kåˆÁ>ø¿ÅaQ¨ô?4£ˆ.îµ?)>|K;U?Ü'w'?‡>Oà¬ÂZ?jjˆÁNy>?i"ë)^¿?ˆ"æÏÅ_!?"`±Ÿz?ïR ‹Ñ/?}ܐýÒGó?|Qè,f?dÆÀ–xõ?/Ž¯5?y0Ÿù8ÊO?ïXág'pK?…°†ôe
?(&ºCž`¯?)®ð
kJ?"³…®C´?…œÖ¦D–Á?ïþŠÔ½Å?Íê  ¿?ìõÙfºO>÷µgmŸ"?#}'g×?÷ØÀ"À´?ïÕ´|Ñë?m‡õf ÖÇ?U´ÇçB–i?R&4äåzŸ?oq"zï!›?gÞ2áÓÛ?ïªÎcŒU?i«èþrh?p‰>'œ§ì?TÁÑH°?zò~E¬?e´E¸bß?ïÙ¿CÍ4?b¿€hXž?r%0A"?ù£?˜?s6<1Éx?b¯ò˸AGN3FGL J0045.2-3704@s`—ÿ›V2ÀSý£¿ø¨ôÀ9x/Äé©|À;êöÃ@\¿ää†Ê+@¡aÈ
þ@Wºßd¿åþóX¿ç'¨²¢eV¿å!¢qPòƒ¿ëGóëZè•AGNbcu?ïø­èÓ`?E…iª©H?0âôÍ?,ԕQ"…H?D×IyÓ?Aåëx|È?ïœ Àûï`?‹™rW`d?eyò'3?|f_1H4h?ƒ´O®æK?'
KÔXù?ï#LÎîBÇ?`Ür1ú½?‡I¾cH;è?r‹û=Nó4?ã
Ý·vf?xn'òÅáŸ?ïÊ·¥.‰g?vèف4ú?'×ï7m´c?7a:ˆ*iU?yån
Ÿî)?vªf¹Oû?ïûFMÓX¾?@†/èÁß?/b~6X?1¶ÿG8Th?6T_o>ÿ?2²gý×?ïÝÇ­—í?pN^›`€?P²^9VÅØ?Ršíc¾"ì?iß#mÒl?iz|Äú?ï†pDΑ?t€¼y%¯_?~!õ×ෝ?d¼D ?µ?~¦	i‹3û?o?Jx^2~?ï÷G{®eó?VS['µi?˜¼ÀPC?¹µ{Ó¹ñ?PÒóÜŠÉ?V,—K­EÓAGN3FGL J0045.3+2126@^CÀh ÓÀD³° F\À8Ú0òçÉÀ;Dþ`Ï6?á!€:ÍÜA@WÛ÷âû?þbw¾þX
¿â'T6@·^¿áOC¢Ê£Z¿Òøx‹›ÃÚ¿ácuxۑ"AGNbll?ïð٘b7?QŽÚ}¬T?C'$'£?<ƽ*néè?V¸åÒõ?JD¯îÇA6?ïFRl*î?˜ÿ†N?wmrI "T?t…™•'n÷?™[Ù&Ò3?•Ñíä/Ñ?î²aÄZQ?"Äλ4U?Ž8(¦Âk?~¥bùh?š—Ç´€V?‡¶&ˆ£ÿ®?ëÄ©Šõ?¥?e›>Ò?'‹ó¶?€T ¾k~?ÂkåaHÌ?¥ŒB%Ë?ïölŽº{?CL›=±Ì?831µSl?0R¯ä¥¥?J4/,éì?<{d³'¦?ﵿ\Q'?{÷#
ѓ?c׃jÉC¡?]áSâ ?{4#¥ÖÒ?x4~ď?ïutpë$§?}`Ûâ?}à"Ihð(?ppîãH|?ƒ²Ò ÚTB?s&™I£C?îPóµ;X?‰æŽJù&?€¼ú®D¾ü?hçC¢
?¦Á†Ðõ?‡"…ôוAGN3FGL J0045.7+1217@^/l?Ä;.ÀIG™¦5À9AvK¶·¸À;n T3]û?ÀŸ.—@ëáwÔ¢Ú?ÿ[@š$¿¹W)˜»ßP¿Þwa¢ÿ–E¿à%Ùºµ·Ì¿áͳiEá-AGNbll?ïçÿ»Œˆ?]ßxï›?IµâÏD2~?BPô5t*?a'ËÊÈS?Wp`o–?ï$J–7už?œ¡[³C´—?v¼,°—u?|SîØ¥õ?•ÇªkQq]?˜DêætZô?î½ërv·d?Œ"·Ã†?'qn‡f?ƒæ>±î/?–Ñ#.ê_k?'q<°ðÛB?ëÝxá4°-? BÝO?',Œ¬£o?vˆýÈHÕÆ?¾Î§vÅæ?ŸàÜ;d6	?ïö'}|"¶?E|À߸?7Äõn¤?1"<¢ëûX?IØ")"V??ÜyiûÎ?ï¹ßgY*"?€y	—'ø?`£p§AÖÅ?asaqk?z¾"—þ´?|%þã9'—?ïhŠƒ"·é?{êaˈ'S?''H˜¶Í?sš†*³Q?ƒZÝÚXÖý?q:ö¢fxV?îÂçӅÅõ?ƒR¿²$X?q¤U?»—q?Ygž&ˋ¤?¡œøºIJ?'›~pPN'AGN3FGL J0046.7-8419@rñŒ¨À@gM@$³>À9Âw»ù?òÀ;¤gHäu`¿ÛÖ'/€‡@'ML @¡€mΐ¿æ"œã·0?¿æŽ8'm«¿ë!ghïؖ¿ïÿŒDÇZGAGNfsrq?ïê–,/f~?z¾*+"q³?WØTÂÑa?zŠëþV·¼?RûR«ýT?MæD·ñ?î£ÉŸ‡½?¤2BË?…0€ÁÕy¤?‡I¶RC? wFòþpÑ?¡9ò¿p?ΧdÖ?ni/½‰˜?—Hvö³Nl?"—†yî7?'åï7ϲØ?®€Z})ï?ìÌÅ¢ÙU¿?¦pšà« â?œgýŒ4?˜
›;9¥?²€
ª@8ˆ?¡Šeeˆ»"?ïÛ­ö¡?«£õÂS:ÿ?o…>f—·‹?«¨eöö?E¼R†ˆk6??³9
:å?ïŒ[õ§Ñ?‰É¦ìWE{?oéÐ‰??jAÈû›'#?"î¿e]^?…»J¡íX¼?ïJRî?z\×Â\?‹÷RqçÝ?sòâ?süËpíÛ?g¨*t©ea?ïBäJ ?‡çu¨JLÚ?qý»Ç‰Éo?sï[ë×µ¤?"?Pä]³?…‹^S®AGN3FGL J0047.0+5658@^•[á¨&$À"›!
À8¹R¼ev|À;\ êƲ×?×
Õ*ŒF@=ijý¤Ü@ËC =͖¿åXûRWvñ¿â4Ä¿àR+•:m¿èvK-GXQAGNbll?ï'è«á«è?"Á‹K!%?tM²J y;?uÙbŒj?ûàŒûW?}ïãM"æ?é`<£ç?Æ'6¿s?§uÜF¯•C?§±9è;å ?Ä%ûÉU?"‰5.œ1?íð ãvC?™Õà×!¸­?—·˜ ÞË?Š¦\G?ó?¥"+ÿÜEp?'«W
+W_?ë{ºkKR?§ÂÎ,"~'?kÁ›õ?œ©Ò"û?¼Çf4×
?¥oêíD?ïÝj"b<?jLŠFé<%?^s«
ì«W?`ÛO£šd?c¯¿ãg¾_?^¿­zX(?íáL6ÅJ?±èav:†?'wdÝǓI?"F}©(KÜ?¨¯Œyd^¾?ªã2‡2u?ï^ûôé³?ƒ\Ïæ¿Ÿ?€£Uuùd"?v$	a?‡¼«™*ÆÄ?|G¿0?î¡þ|-?‡o'º?‡Dª‡†$O?rDRà5«ý? 휏¾?…¹,5²AGN3FGL J0047.5-2516@X`ñ7ÀUüæ?Ïù¨À9yEi–œÀ;¶T¶"¥?À7Šïuq@54wž@ZVߊ¿Œ¿âd+Xs^œ¿åFÝA¿Þëqø´1¿æ+
:¥"OTHERsbg?ïè	"àÍ?eh¼^?þT?AÒ_qR?@‰†'#>a?c¯h«§r?b®•žÊj?Ř¥ÿ?"Í":7÷?q2**f'?€sÙX±?…÷¹"ȳ?ŒaJÙÔ-z?ïÁ5²?†Æ󧩓?†PZz8Å?w?ÚSҞÌ?"ÇššáR?€‰2ö5*?íF…ÕÜ/?£Rò%­ÖÁ?{¼ˆÃÜ?tÒµÖyf?´+MÒ?¢ªcæ5Qç?ïø"íÚ}S?HZņj?/ñ4¼­ÿ?,â–üк9?GÍ?%ì6?CÍ7¼º?ïÔyE?€+£ùZÊ?]¨f´¸?ogw Üí?m²bÛÇÝ?s³D©ê×õ?ï•jÜ~ó?tÈ,쪈3?w­k`[Âl?póŽ¼ù÷?}&~0gë?d¿¹q+ãr?ïV…ÕoD?~^«mìÁ"?jÏ;ËD!?Xr"¬Z@?'ÕbÅ™ø?|™íÔ½²­AGN3FGL J0047.9+5447@^›û'ÃÀ $y?ÜäÈÀ:<‹ÂAÀ;ªU‰ŸP"¿Ó"m|҅ì@.‹@š?õVtªL?îé£%o·Y¿ç²õ «†¬¿â?ñÙ
s?á0êíZr#AGNbcu?ìñí
	'ò?µ\w2éÁ?LBªÀã?L&h÷<éŠ?¸8Dj?µUºZz?í˜?åPž?¾g½ýî¥?"ý½›Üˆå?Œ_($8#?°žI$Ýt?¼]>®;'?ìí…$Ó°'?ŸB¤J¾
?žå'1~D'?'"©Ø@?°ÚLÈ%?›r›ÇÕ?î'|,©à?§º6ڏ?>¿ÕŽ?R®KHýñš?¦²ÆÁcð½?§«»ò>^P?îá9ÞW0?§°f®'³?I8ª\}Ü&?NÑKהl"?¡‡Œˆ±aY?§ŠF50Þ?ïlxE$ç?™õp!S¡c?nQ§Ð¢O?€ò»Š]y?M"³§Ž"?"øv´Ç"?î
PqÌ9ï? Lڅ9hÁ?›þD<e¤?—±Ü‰íÏÞ?¡+ÖÈy+?"@
َ+p?ïǗ¦¥EÊ?yz»Ì¹'?æA'ì[?2à|›…^`?{¼"¾3á?y2æX iãAGN3FGL J0048.0+3950@^Ž&áY.À7$_ZÙjÀ9ݏRîº]À;¥e5
ÿ¿øbf	aÀ@×)_õ³÷?þna«¿Þús&pà›¿àÇLÏLÀ¿àc¯1±Rô¿Ä30×ÁÐùAGNbll?ïô奃)?UM2"þ?'4üÅç^?&£P*ö«?U•›!Ìá?S¯2';2¡?ï'XÆä?ŽD‡Yªî?h[ÝÑuá«?jšlV+7?…£ò\*,·?Š§@ƒû8?ï.ôòÕ?'þáâù?',—Ãï™,?r`~ËX½?'&u"2ªÖ?|¸_Z´§?ïĒN ÊP?vi­h}º>óšS¯sþ|>ýN9§'>5?}£>­hš%?vf­ü¬F?ïùÉ÷ýŸu?B±;¬3´? ©1Ø÷ÛY?!ŸZ>ýô?D­Ó"…e?>˜ªxØÕò?ïڧͨ®¤?kÒýñæj`?R¦J‡Û¨?Q1´Ý\±ñ?l^ù³ÖI?f0ï'?ï¥	ñÄÝ?rÃîF
 £?r‰;£PCé?izŸ¤ə?zñËÊoU?jÙm0YÀ?ïõod«•?G~7A"¢>Ô4k¹Ìn¡>н[.&O?U
¹mr?GvXâú…AGN3FGL J0048.0+2236@^z)à¤&ÀD!Ðß´0À9,ƒöš%±À;™!|QŠ6?îá¾y!ÿÚ@îþj(½¹@ª  žŠ¿Ût'冓>¿æ¥ãµ$B2¿ãíw3µ‡¿ë/EcškAGNfsrq?ïìT	|?Zu
šR?V99{?R‰Y>ºm?QVÅ5¶ª?K'^QD&ð?ïz°V¹9?†žËE:?k'‰±#¼?l­¿Ð?ŠŠÿs€:?'…wù㽞?î:ÌÎFÂ?"ä:º"Â? ‰ÒÌø?×ÿú¯Z·?—'ÒÂU³?'¨ °'½?ïv¹O—lï?‹›ö/
žX?^Ã$ŒdB?e#ó‡D*?ŽyKr#›×?Š\r'n?ïö݊	XÄ?F¾e~#Y?F:¯§‡E?>¥¹,v¨?<žN¯wC?5MùÑ#8¾?ïφ«ÞÉ,?r=Í`['?Yé'híf5?U«0¬°v¥?qÂEz˜R?lƵ9ä?ï1ƒÔÃ?ƒð½)-+J?'E¢­?VäøëI?"†ãÇU¸›?q="zŒ³?ïãW5ÏxV?g³PŠÁx?OFè…a¦?CêÅ~œ ?d×E›‹n?eUfµª"AGN3FGL J0049.4-5401@rùm`ûHÀO6@-íyÀ:}2Ȫ(À<Çhß½j¿ÿGDAùI­@ry-hmþ@%µ\Í¿æLÝÏ\&пäcieŽ¿ßúÍì\Š¿Ö ='tËÉAGNbcu?ïêßïF?_"ÁnN?­M÷ÒÚ¯?"P?ÔÁc?d[Eê?^«g+Æþ?免¤§u?ƒpéšyP?_l I†?bFÚ:¹±\?ïiˆC€¿?€U'Ha?îÚt®[P;?†ìmþ•"¨?‡0L/֟?q&E"wáw?™D"-w>?¤mtÚí×?ïÅÉژ×?tØ-Vñ^>øhíÅ;5Õ?ºbËGng?}©Ê1›'?tϝVñ?ï÷¶û<Ì?K7B%iڕ?´u7O¢?
†Í`YÖ?Nƒ¥éÔ?J4ø¼ò¥8?ïâ}q"Š¢?i4š&2tì?KãHæ™?MO!Ín?f‰¼{I¹?cçäBÆ·R?ï…M!Ïf8?p/_Fh|?w¾K,V?bmK%ûä©?'äØ]¬ßï?gb£#¶1Ž?ïöçï×­•?G±báˆJ>Óx×…U¯>ÐÑÉ6\؏?R§-¾m¦?G¦UÖ®AGN3FGL J0049.4-4149@s[6†¥ÀRÓ@ÃÀ:–²gƹÀ<"ę¿Û;óv.Û`@­"óoMì@<zßð&¿æðÊ㓍¼¿êöÇvõֿʪ 1'%¿È9[ã¢ô"AGNbcu?ïåÕ¸6p]?hÀqeÐ?YÈz¦/:?yH´ÉÂ?i/ye׫9?gãݨÕõ?ïˆ?Hâ"W?"/E(XW¾?hl`UŸ&ž?w1Ö¸C2ò?‡Õ·Š¥?
OÕÈwg?îA­çPÓú?…´CðÃî?‹à±Ø–ß?vðÉï1W?¤ìõ… ?Ì7TÎJ?ïÇQÛv?"¢(jt–j?8ñégúÚ?EƆ<)\?Ÿ#N#Ó¾?"˜Ã¾'Èw?ïñü°{nœ?Xñþo½P?~E2? û5W(Ë?ZW‡PÃÉ?X ¾+iN?ïٕIA¬7?{éF!™Ð?Sõª‡ï Q?dÆô™ŽÁ?loᮖö?rÂÕF}Ƶ?ïDÁ^•È»?z*E¿úñÁ?rCªQà?iéÞð)¸?ïEo6I?u`—²@,?ï×ßZC'?hVßNöXp?*_X7åf?+	IýØ×b?s;hró?gÏùƒàÝAGN3FGL J0049.7+0237@^…п "`ÀNJÀ²¤À9h"t¼À;°â`²È?'ãY,@è(©c@óËßgD¿ã,ï!¿äºjþÚ¿Ý0r‡B:¿è<IiÖ]oAGNbll?ïíëÎi@?_BýÓ§s?5ߪÈߎ?6¼Ž³A	?^±ãXÿœj?\/ðz%[ì?ïs-•u®¿?£½Mš^?mÏá-o¸i?|úÔьÒÇ?‹À¢`×J?‡Z³ˆ`À?îÿ'q=@9?‰!ÛòÚ}?ƒ…KJ(‡§?o†6××¾«?–K,9žü?…'V"Ý?î±úk–|?"ÍzæˆÝ?c8³/ÙÀ³?a"éÿ ¨µ?£¬ÎJÆ?"5¼Â–ýƒ?ï÷ L*ê?q#5¹É-'?)Ä9W¥»;?@z¡eÑ¥)?K
ÁÊüÖÐ?n«7~¯É?ïÐïå?t¬£–+}Ã?X3³YˆÛO?V±ùtÂí?q{‹*"Ò§?p¦{Dèéî?ï ¶I?r±8±GAO?q ÅT¬ÙS?W‰ˆÍj?~U3˜Ê+?p¬¿ÇÆÊ ?ï¹oÇ?p%'(Ì¡?P,·gø?@ý‹ÇÏ?@H¸u?ní×%³SAGN3FGL J0049.8-5737@rõœýç!ÀMÀR@>´qÀ9ҝë7òÀ;ØÌð;8¿½Q‡Ðw@‡ùZ"z@²'€Ê÷¿èà{ô-å¿åòˆá±O¿åîôŒÚD¿Ò®D$ТAGNfsrq?ïêZ"v7?b©5H*Hû?CYüº{¥?B~—¸65?`Î삹Ê?`'n
¤ún?ï'KúbŒ?èɂ"?hu Ok!0?vCà§b–‹?‰O¹Fu>Í?ŠÄC.!?îgCXoWÒ?'¸[^rš?'«ý²8p?z¥Åƒ£ª<? ÿtw±±?‹³Ãç?îÐ-†(×?"²©lÏ?]ì_:dã?_lÃJ¶"@?¢
ÊIl?"©ƒ¾ÞD?ï÷¸™l«­?Mó¹ïÍ?0p,8Uã?-ú{0/~Í?HåƒÀÿæ?IóTÊ\5?ïÙSf났?nj&}ÚÙ¥?R̓K×?RzüpŠÈ?mE×ÉTÆ?h`?ÿê?ïr'‡•qR?rÏÿ|åhV?}¸]ež?aYœî֔y?"Ü'ëÖ ?lþs ¨¨ë?ï͂R2ÛR?mIt-zí?AªòÉjõ?9°Y8˜º?w	xu™Ì{?kïA9°Î³AGN3FGL J0050.0-4458@rû¯_Ô{îÀR	â H¤À:NÈ>Ȓ«À<Üq…~Z¿ãP€èa—Ž@è«,¾úÒ@9Ÿ…@ò¿ç³Zh‰à¿ààêZɜŽ¿ä*NãgîÒ¿ïÿ—w«];AGNbcu?ïí2'›Åæ?cq-6;r¿?Xö€Ž'×?aÄ«Lh¨?IH´O¶R?EÆY§:Ù??ïS¦•þ?'ä.¿æGc?r&°¬"bÌ?yi5hŒšN?'_
Q'š?Æû©8…ô?îòy'û?•5B€MÛ:?£p·(Cí ?'šïHçiJ?•àB'¥V?'öý‡±½?ïì/ØN¥?ü&]‹6?pâõ'úÛ?p_~;Ttã?™‰¼½ò$±?Žé3qÜ	?ïöUDz±™?MH?v¼E?Hã³VË?GP×¼ñ?;Š]ù®\z?5†)|;?ïŲ5ê(?X\>Oµ?_ŒH&x"p?a*Š@ØÜ©?uCÓ!¤7Q?x§ÇM%G?îßÖ$}?Ï&'30?™$±ÍHé?ˆ› ý2'œ?…Á´wSd?w=nY;Ç?ïÓZî8,l?p ¾í·6?K*íRޘ½?R÷*nÀ‰g?rí+Q}Ù?n++—¨f³AGN3FGL J0050.4-0449@^"¤as¸_ÀPìû_ò®ßÀ9ž±ý=­àÀ;§Ôî~:¿Ön>ڎà@'
ǾÅù@™\ÀJ]q¿á—:f®4Ü¿æ"Q¦ùT¿ä@Î>p´¿í"Ó_Å|AGNfsrq?ï¿ej+ܗ?È"pÓ´Á?x7}i;·?~!Oœ§–_?`+›>&W¶?WŠüeq>÷?ï'â–
?œDÌN&ó?{+â0]':?š…r0L6?—RU5²+›?˜ÒPR${?îEü~k?ê?"#=•äb©? O'Ó@-?<¥µHÜ?–¡J…7Ìp?ƒ'êTÈd?ìiª5ž‹?©®!¸wÛM?…ó¿<ÜÎN?«ÐËÛp_?¹ô6nãØ?¨¸:ÄÁå?ïÙÂVQEm?q'qõÏD2?koklc±?p3'U	ù$?Uœ}$?Pô*|³?﹁–÷Ž?|¦¨"#?cœ¬}/ÙG?cL˹ÀK?ypÞ/çÌr?v&ýèÊ•?ï!àÖÛ?…ÁöÕÀÙ}?'ÍӋl€?—Íþ"aš?ƒìU(¨w!?pûÅì|?ï#¾ë)??‡':êR<å?gԞzñb?bɜՄõ|?˜§¡ê×ìê?†JÒ(«HAGN3FGL J0050.6-0929@^•-û¹ÀRÄ`Á
À7ï;M;À;
;…è?ÌÚ#ޒ®)@ø‡©'ö@¾ž²gÇ¿Ýè%Õ#¿âËÿóγ¿áíT<ÿK¿ádiÛ±ÖAGNBLL?ïùü~HãÒ?F
}ԖHu?
7Š¬Á?̙ìzã¾?F:ŽçÀX»?E"þùXP?連­"p?"èŸp†|?aF¿l½ô'?eôú—! Œ?'ÌDj&à?+û@[š?bÒÌÛ?•Âÿ×V·ž?…O"'η#?{‰Äa‹ç?¡áìg¶Œ?"êŸÙj8/?ï~1µÉiÛ?‹ÈgÇÁH€? EÃa"w?,îšE!B?=À_>?‹¹k֊ƒ?ïýÕ_\JÈ?(o.ý³ù?
æ8#_í?ê7ùo?-f"<Òõ?&dW§5S?ïãX0©t?h2ð*:ŠA?LY–•?MR«T›?e¢âQö?bŒ@r[!?ï;aŒPʍ?!rž@
?y{栞s±?u$W¸¯?'4Ôц£{?ŠhTR<¸Ã?ïá.¡ï?eXpÕ6E?óŸ¿Ÿ?©ÜBÙ?nJb'"ñÿ?e9ÔFÉRAGN3FGL J0051.0-0649@^ª`4óþÀQlÆøÀ9'Þ³íÀ;€X‹Ž>?öÛ)üþ˜Í@]‰~noõ?þôwÉe9@¿ÛÐ\ùпäñÕøO¿åwåiÑ«¿ìh­ø AGNfsrq?ï–ZwPØ?ƒÿ+7q÷`?ƒËr Ù™W?€î¾×"Ì?jw¾¦b
§?h©¬†Îi?ï‡5j‰Ðh?Š×f}ý ?gDy9p`?kŸvJ†?ˆa‡Ýù?…ÌÇÐUñ¹?èŽQ~š1<?¯zãÃUÍ?Ä:S[yù?©
lR£5Ü?³ÎãÍ5? <.†Î?ï–ÄŽK?•ŽÕî?q&pugš?sì;pM(Õ?™Š]Ê2)"?"Xº&8I?ïÀBþW^a?{C5€0º"?z6g·žŽ2?xÏñonwØ?V dÔFY?Rq>>#±?ïÐy¼H_?rþ'"V?Y¿¦©6—"?X˜6êæ#ô?qS8&""?k[Üâ©	?ëEÍß=à?ªb>=ÇC?ºÌGÁµ—?¤¥þd›÷?§—‰€0¯?š AÜÞÔ?ﺾ¹¨q"?y Î¹Û\H?g«ËQ,F?a$ÖþÆÆV?vʽ­ü‡?t³¿&õKíAGN3FGL J0051.2-6241@rïj_"ÊÕÀK8X R…ßÀ8Ô¢ŠÙã6À;ÝS¨?ãiËÙìÙ@SBïòÌ?úœF__áè¿å.w†Á¿Ó3h7Kñ›¿Ì{fLTU¿Ó)ÈÐ,ÂpAGNbcu?ïæäÅ´L?]¤Ku‰§?NŽº¦¡*?FRá/¬\?aw‹½cÿS?Vå½~t?ïm!àqè?ý TH׊?oœÌD2Õ*?v5¯*Œ?ŒØ"k($ß?‰F~Ì÷R?î%À™E??–«'¡z$?–Â_Ð9Ã?ˆ:RÞµˆ?¢BÏÛ»v:?g¡?yi?ê2ü;€µ?±ãWìý¤?w­ë0zp?z†1Yמ?Æv¦ÿ¢{Ú?±ÖhùÈì3?ïóÑ¿¶õÜ?LNT֛?@Ϫää{?7íŒÏ6òé?OéUû|f?DÛæå>rÞ?ïËz­£ÅJ?xÊ-æ68?YÑ|X9T?['ÄžˆŸT?sÎa­[ Å?tójE–?ï'–ÄÅ?‰€§»·	?ˆPˆàb Ÿ?ÉhÝÇ¡?ÉÆí¢K?^Ýy£ö?í±Ï*¡O?–÷öÓã@?~ô`3S?m4³úb™?°j²šT?–>Ý£n5'AGN3FGL J0054.8-2455@aÐØ`fÀUêeà.©aÀ9G±CÝ¥À;Ph¯ìÂ6?ÛgÓ`¸@ÕÄÉH3?ürå?µL¨?íš®t>Ž¿Ýb=ºd¿Ó<ؘ£Ù¿àtuȯAGNbll?ÚÎñ"DC?Ü*¿¥á•K?O±/«i	?S\Fpê[?␚锝u?Ü)²,Ñ]?é
k•i"?Ö1i¬ï§?"r֐µºK?ÚœÂs?ʏ$B!)?Ö3I•Â–à?éû")dl*?ÀK9Ëcý<?ϧ?'wbuµ¡?ÆÔ^øš?ÀsÓ€;Ð?æ^‡+Ð4Ù?·!E¦ü?Š†^ZQ¥Ò?†³ãÄKy?Òn¾µÄà?¶ýá ?×苻pÀ?Ý´†üQÇ?0Xž#4Hø?Hó8¯'õ}?ä	¯Sˆq?ݹ,µaB?ìđúéÀ£?Í¢ŸoÏú1?t–ý
V‡¦?‰Í¢ÔŽ‰±?¸'V¾²ì?ÍTHŽ†p?ê±,Z¦ê?¾³˜;~8ô?'Ï+"Q?u ‡*žgž?Ä¢Ùx?¾æGr/r^?ì:TƒÔ¥"?¢'xÄá?…›ŸnŸå?rÐNJ¢?»Šˆo$Ðð?¡ºՔžMIXED3FGL J0055.2-1213@_ ©?)
»ÀRÄÿ¿ÓÀÀ:xHG—nFÀ;ö
>¬ãù¿àÓ|¶¬F@ìŸf7A‹@,€0¥¿á †N
!¿çÖ´ñӆ>¿äü—öV^¿ÛºßáÛíAGNbcu?ïúàãÒoE?<·²‡þü?gÁ"O°&?!š0=þã?@wýîË ?9kû¸«|?數8â¹b?ƒŸ»ùÁ#®?`\{ŧ?d\ø!»ñÆ?'~¢1 ?€ùôkÒ?ïf0KÀ?"r«žŸØ?'é"qÿ™?néÝ°Fµ?'ÞwÁ˜ì??|níI?ï¦êÐmì?}5xö·?#¦HÎËî?'`L_íá?…ö²¿ÔmŠ?}|,•š?ïýrç©?-_«}:?D?}V­ô®?<ÝRÅ?/'øT"¦x?)ˆŽ.M?ïáWpª7!?jSñ¨…G?N	1nC?PY€Bv?g&GÍ'`?dwkbIÚ=?ï§ï'õe?hÑ®ÍJ-›?q7;¢Ê?[eÃÅr(?zÐúÓ¡p?a˜½Îª¶?ïñ²õ¶%?T*ŽâUd?́vb?@ø×Ñ>¿?[›´¯'$?Sà£É¿@cAGN3FGL J0056.3-2116@`½ë¿×ÀU
€!"À9•ÄÿxñƒÀ;vÖ
c0Q?àÙo@`Ö#7½‡?üí~@!Ù? ïÃ
J/¿ÒºJ†-x¿ÛÅð Í§¿Ù×RH'ÖAGNbll?ïö 'Ó-º?FP.zöJç?:‡¬`)±Y?:ÓÄi*?H;Š§|ì?;àÿÓ.‡?ïec(2=?—ˆ´;}Ñß?nîO¦ Ü?#Žrò'h?ŽÿSO
é¹?"ÛN%ð?ïi÷5ù?‡{žwrÿÜ?†Õ ø&¦?woV‰'?'h;J%_'?'F†áSí?ìï̔vLÁ?¢<ŒÁ²–?r‡`°?oÓ4½ß2?·Y%YŇù?¡û È!—T?ïúL?|J\?9"ñ÷ÀÂÔ?1~ljÆf?.£2ÐÕ?<Žƒ·{ܞ?-†^ë'Ü?ﶜðÍ?'&
´â3?Yfôàçª?\§¹qú¼?xg—±g?€"ÎJ§¡K?ï*†Ò?x¿Öw(?|ü÷<ÚøD?r1J6L?|mż~~?lç‹AÖ|?àÊI?'팉0'ä?jéÀqùXM?XÔݼ?™±Óû~á¾?'<Uºª\÷AGN3FGL J0056.3-0935@_½^	ÀRSÍ$áÀ9ÁÕùµcÀ;|Fûg¿³Õ¥½@8@7s'À?ü¤À Áìt?ìÏ96Ç+¿Þ$ÖxQ¿Úç0‹c ¿Â^P»HAGNbll?ïö'a÷I?EºÓ*Rò"?1ӂ"ë?)Νus?NÚ‹']?B%‹Êì²)?ïšÀ}´
ß?‰<֍$r#?cÖ*tŒ‰?s/»àèvð?"Z]xéç3?ƒy1õ'8?gH?""Å*‰Cö?…vC®J?sæ®m	Ç?'ë²Í¼?°ùŒ
^÷?î+‰¶w Ë?œÄFy2²4?D8Áï;?Iœ	|¨·?¬ö'
Ð?œ¨G=sl?ïû\©h•?6t²1;V?!ñ…I‰Õ?!5Ç*KND?<"4Pip?0fç:©á*?ïßEž«ãY?jK­Åûî=?P
I~=?PrŠ¤Ç¿¯?hµ<ã:?d)ôíë'ò?ÌXÍe?uØii¢D\?yô­¨ ›X?n¦Íq?€×6Ä:ù?lqÀ‡#0@?ï"[eÆH?z­
ùyò>?6,ñÃuð?1zû ¿D3?Š7¿c¥?zuô,C÷AGN3FGL J0057.9-0542@_ÖNaŒâÒÀQ!ŽèӔÀ:43#Bû'À;¶Ï†»p"¿ïzI²‡@,
{®÷û@R²à£¿à¼‰ô
(x¿æÒå•Ò¿å_ï˟J¿æ¤´ïz;AGNfsrq?ï¶l­Ê o?žDÜxpe?Qíì]o ?RßÔçým'?€'$Xc<:?€ÑƒÄÊd?ï€"|ח?åÉ7s?i›ìí?x€4äP["?‰€–=n ?†‹lXŽy?í†ßÌ?'?›@øÑ_?œ'.uœ*?jÍ>¼È+?©":#ËÔ?"±ë¯°?íì»ujÿ?š)ÁØBšÜ?ZÔi1pˆ?WÅpxh:Š?°1Ù²"D?šîÀê×?ï솮…d?b/Moÿ?61ލm˜y?75]ûñF?`³hâ_Ž?`ÖaÔ¸¨?ïÚ€'z?oY¼óœ?S¾U+þ¦?Sl qZýO?l["{VF?gØ^A§Ø?ï(,4økr?¼\§9?‡Z;ÍÅø?z¡RÖ}®ä?Žg˜f1f?uBqåâÅ?ï‰GœFj?v[çÄä8?:þÁaÐK?/¡+qÖÉú?ŒÖ"í?uåœ7¥¬AGN3FGL J0058.0-3233@r	€bïÀU¿ÖDEÀ9C'5ÏÆÀ;€Æ'—¾?ï+I˜¶€ì@¢Ž>F·Ÿ@w~?ËòÝ¿Ü«#ñ2¿ÞšMìût¿ãX^v‹€/¿âm+©û~AGNbll?ïçhµQË?]üEoz©?NÿvbÝ?FƒL¼™‹"?`Ø‹‹7?Wˆ\ڝW?îq¢C®¢ã?±±Må•?‹Sû?Îb?¡üŠCŠ?¢
'a8?¦Ê4Y2})?î‰ÄGÿ.Z?"ì—XÑÇ@?'ï;¤«Ls?"§Ý,ªþ¨?›Ø;`–RC?ŽCÿ?é¶6
±'g?±•«[£?¢añ)Öñœ?—}:‡H/Û?Ď«‰±=?¯­x¯ÐMò?ïôUÚ½É?Jäö?AUÐÄ<?7x|ÉkL·?Mš§W
«)?AD|Y)£ž?ï':íºÐ?ª
*ÒÕã?5É¼?'åRÌøãù?"KV1éEÏ?¤c;¦®±Ø?ïkÁ8]Ù>?'‰Š€À?7¾B{f²?u}â¨?ƒ×ó¡>ÕÜ?zÏm›Kæ×?íì±R.1R?•
r%Ù¥Æ?–Ê R?Äuôµr?¦-…ÒÅè¶?'†4æPQ]AGN3FGL J0058.3+3315@_%þKZÀ=•2¯ÈÀ9ή"i›À;й!õN?ÑÞüûÛO@ç0+kéˆ@B"@Îé¿æTgê䩧¿â.ñ°¿æ[š6nô¿íËLŽ'JAGNfsrq?ïƋŽ­Ç?zÍù‰J—U?xEöh—c?yIQE7š?QÔÊL]ßV?Ljïe'¦Â?ï4åõ'¿?–T‰"(?x醧°?@æ¦oòS?"BÛg‡]3?'s­"—Âo?í«Õ±Lé"? ŸB]Å~?ª	%ûŽÃ?›(<†¯aK?–r/Ôª2?†1ÂÊßD›?ï:Òýq
?‹à÷%b{?vpÖQdÝ^?o(½'Šð(?"	jÂ(Ÿ€?‰|}%°î¿?ïÚ[çÄ`?qY-oçÏ?oþ֖ñdÚ?pu-ųC?F•õן?Cc× Pî?ﺼ`æA4?x•°{geN?c&"r&~;?ZôC¼ ã?y¾6?'Ñ?tüß$˜Y¶?îÊ><¦¤o?á˛ü¾?œQŒ¯y ?«rcv|?"Î7ʶ`é?rGfðÆ	?ï×ò·ºc`?f©-CBh?[AÃèwK/?H$\ɝ¿"?jlfBB²e?dD¾•æRxAGN3FGL J0059.0-7242e@râR€jôkÀF5W¿ÚvÀ7îjCj¹À:ô‹…à_?í]ñg¶È@AT;9½@đ #a¿ÛÆ2x'É¿ä•×m9¿>¿ävôô3C#¿è"äÞ¼csOTHERGAL?ìR%Sn"?³+ÍB¦^G?­*˜##¦?«ô·DÌÏ?­³¢5GÖ?£ó&*pË?Ý?#üßd)?̚ÉÔc³È?Õgq†ÞŠ?È_ŒA
ß?Ë~é#3z›?¿(ed]͑?æ‹í"°Üà?²8ã'n?Á~ŸÖ}-[?¨ìkã"۔?ÄQª¿_&?¨87M¢ñ?ÊÓÜ<›?²ì£±êV?Ó±Jm±3?½"D^»?ÞäÇï‡%½?½ŸU'¦?=""˜?¥¨¼}Bw©?•–«ùN¨2?£u,3¯?•ô,Tu6ß?)¢¸<¢?äTZ/ve7?ʁ[TyZ?Î>²$L\ò?ÅLÝ©=üe?Àoå´L´?¶PSòžØ?êAH^,tí?ª¦ï2v4?¸èҟœ(o?¢‰9',nÇ?µêpJ
¨? ]P"ñWÿ?ڊíß´u?±Oqa<?ÍÔÒ|Ԛ?®÷`Èbqõ?֊©äaá>?²\tTÎMIXED3FGL J0059.1-5701@rÍÆøÀN	T9À9~@¡°À;ÉS¿šµ?î°–7@¨•žÃû@îpnö¿ÞTíPo¿ç•>&þ¿ëH_TÉ¿ïÿåώY[AGNbcu?ïZôa€w?§‹"hrW?tX¨Ò`yV?{º(?"?bk…?¥¡rÈG͌?çÑ
^®Y?ôO<ÿé?¿]²kUA.?¹U)fcˆÒ?ÁòtÚ¦?µç´Ä==??ìÊVzWi?¤&@kN?«€ˆòœæ?˜ÛÝC¹ÿp?§Úg'e'?™Æˆ/Ñä@?ãŠélY‰?¸¼‹ßÐ=M?ÑÜ
åúN?µ1TÝc.4?ÁZ>'¥??±
 ´-?ï˜l"9·? }3kï?j–NC?}©¦Žý¾?ƒ?Yšm¯|?™"oc:7?ëx¦‹UÅ@?´qÞUœ{?´@ÛRѨ?¬ÚµÁãý¥?°"ŠÈµ)Ý?¡o("º/é?în'Ex–P?"enÍEÌ?^0ö¶ä?‹]çI¢KÊ?"ϱ(…?ˆ'ºÖiÔf?ë–aÓ|
à?¤Ü›jâ{?¸º
I]?œ`ƒ?¥%¦·2ý?›G'}EšAGN3FGL J0059.2-0152@_߂¡/ÀP+á .QÀ:k+D´À;½¦læ³(¿Ô·Qª0"q@ï9}$C?ûÍ[ d¹é¿Øµ{!‰g¿ë´kÏhç?»¹=ìÓ0¿Í²w°}þAGNbll?ïɃF›ð·?z=ˍ°?¢ºÃÝ?¾AS#C<?zûÑÃ黦?z6ȒK3¿?ï¥Ü€ýt?…秋Κ?`ÊÙÊ
¡?cχgÇ?'V)?Z*?'(°ü¡K¡?î{ìökŠE?ñcu"Xq?‰`[Ú¿?x<ÊU`?¡é*Óø–þ?Œ˜c3{?îÞd$í ?št¾WŽé/?'åª*Œñæ?;} Ýä?¢"B?šj
ÆÚGô?ïé±=Û?kÛý'´™?³åœP®8?	FlëòÂL?eÉGÁéy–?kºÁ˜¢^ö?ïàüÇ2Ñ[?mµ/6£O?N‡B½fE–?Rüc®r9?gahWƋ?eþÛà:±?ïKÌ
N?{DßSõ7?~7]£L?o~j˜•Ã?ñ|"Šé¨?tÖcۅî?ïÌÅ^ª–}?j[US«$?%Y;/šR?$'ÓëªÄç?xò†Õz¥ø?j<}öAGN3FGL J0059.6+0003@_ÙØà†8ÀO_Ï¿ÆT
À:J'ÇÅ&À;ϸé?á÷÷ßA'@¢éCÐå5@ß&_3i¿ãÓÕ!&Ž¿æ5h¡Bõ¿çÀµQRzn¿ìŠðð~¿AGNfsrq?ï˦<üEò?sÜçkëÛ?p7´Z&õ?p
ÈÄ_Ú?c뉐ÿÁ?aÕ¤?î«Wߺæ?¡ê†‰+R?ˆ
a°K¨?ñ҂ӶI?žÓˆ'äÚ?™¿‰v_#?í¡X¹æÁ?˜i›Bˆˆ?¢P5æU"Î?Œ|¢X~?£šIŸÄ?Ž/"«œ=?ꎤ§Ö?§‹"¢'Î?«bE¨'gR?—/ÎÁòè»?½Ù¼|ü«?¤ø|u[?ïÅ°}$²¬?¬eÙ§sÇ?v¦µ~Ùý?¬i¨Š)7}?Z/Ë°Ô/?ZÅ1Æ¡7'?ï—Kspåñ?'tH¸Ü?pך¼f?nïõcÌZ›?ÁV¯B—?zuðb¢8Y?îåÆb_G?†€dtýk?"µ»S̲€?¢¦JÓs?"ðӎÉ6?s½-^9F ?îiO‹JÞ?‰fïꘗ?—֗ª?Õ?xW",‰^?›¹Hs|È?ƒ÷4«^1AGN3FGL J0100.2+0745@_°4?¢­?ÀK…à
—3À8«sp:$¿À;
{¬HÈÇ?óîCÍ_CÝ@«wènê?ü¾ÌßAC—¿ÂhÍÿ|Í[¿Ó¾Å4ts<¿Øw=N?(¿ÛþNuÀÒAGNbll?ïéœ×Èz?fúµp>FW?GÙ/u6ë?I¤Ý(D3•?`lÜíaª?c|£âÚ1?ïaÌ-?':ØßxÎ?pá~Øö˜?}úUKr?}[3‰?l–÷ÀÐÇ?íù&êFþ?¤³……ź?¢®0]šù?•›±£…é?«r=4=õ.?žÊÚÝ9_?ëD.]?©"åØa€?†[|')N?"¥ÌöšÔ?Á‰ŽÊË{?¨"a̙c?ïúä…%C[?=ÓÆïUXù?1Êk{'?0ÑõY©^?7Äghš?4p‰kvƒQ?ïÈ?ž?_€?zu,ç"µ?]‡Qɛqå?^&϶*Û¶?t~\Œ%óD?vj¦Ö—÷?îÖh¢*â­?'d	È^\?•ŽRšé1?‹½‰ƒŽú¶?I2@G'p?‹³ªÖ?î#({@µt?Ž5Ý©X?‹=ù:£?vMp¹5@?¦ýùû»?‹qŽÂãÛUAGN3FGL J0101.0-6422@rÓ[ߏG0ÀJ\ŒSâÖÀ9õ[aO¦À;Ê~ÀÐ?H?þÃ	õ¢.@
~×ÌZ6@FÂ5D/…¿Õ€ÉÈ¥9¥¿Û'hÉþÅ¿çM‹È>H¿î+
Ö
áPSRPSR?''"p€µ¹?~*oÌ2÷c?ïCƒ§.?†Å¹}(?sS7uè-‰?tºªëŽtq?² ð{ز?¾¯ºÿ'_?æÑ?øŠã?ˋ˟?Í?˯ï§['?ÂÜ•¶"?°^쉓'¢?žÇK¥è(ë?ë°Ä;àZ?§D—Vð½ó?²ñžUz?EٖaŸ?À¨*¥‰Ö?©:¶ÑJÑ?ém	5çK1?°ë]%õÝè?³GaiÇ=?¦±'?sÔ#·ú"?{={â'À¢?ï³(LäW? ltÅÀ7??r—͹Eû?Ÿ¾qvW"»?À@GÁ";d?ɍmé^ö'?çvžå*^?ÏÅÆ[/§?ÃmÝÂØ#?¶É‹z¢&"?ºqϔìûZ?¤‰Ñ\uï?êÊú8¯¼?«³©æóÞl?®l½Läû'?r©ÑÜ<h?Óñœ«Øò†?°'é;IU?ä–æ5ÿk?¯"¤íS¸¶?¤I¬?C?˜AW?*XPSR3FGL J0102.3+4217@_Eð¡¾+IÀ4‰xmžiÀ9SDñ¡˜À;Â"³‰.è?éSGà¿Gÿ@š€Ê?Õ@ˆˆŸÌ8¨¿æÔŸÚrÊ¿èžr!c/®¿ë…܇n¸‰¿ïü-êì>úAGNfsrq?ï÷[Iãßõ?J#Œ™ó~,?AdUb¾m?B§‰ûãp?A.ƒ÷Š?91Ía_ܵ?쾶¬yñ?µùÝÕàQ!?£BˀÂ>F?¡h"âsY?°häڅ~!?±s}hE?îÜÒ÷=?ˆ'#1h?•8÷Ý
¡]?Ø*TŽ‹í?Ž]+½
¶#?vîŒ3®Cý?ì¥æÑR:?ª1ŒH…ýF?²ºì±‹×?¢öE›Î?«'+ºc«°?¢AÞú?ïï"5ø?•"®"[­L?[™ˆ– Ä?••ÂWOˆ"?5y÷v2Áu?/«ø)6Š?î¸\™DEe? \Ýhc\?ŽÒÁ4f"±?"«LŠÍAõ?™‹6dÙ?™î9qXß?ïG†M¦?ß?vg)W+ÓË?Œß¥,úÓÔ?q£¡Ìõ?>Çbíòu?b¸C&"9?ï´äðýP?/Éàøî?"'q.™Û?|ZCj6?ˆ¥ÝóÜH?‡j}!hÛaAGN3FGL J0102.8+4840@_7ƒ]íñáÀ,Oö¿ž(À8ÏϚ¦ãÀ;MIðäÚ
?úÝÙìD@­AÂ<@œuhâÿã?‹þrى¿Û®Ó朂¿å‡)yù\¿ê-s>¢8`PSRPSR?ÉkèËç?¼_9á$?éáh
8*q?ÀÁ<
rIÉ?£Ãϊ,ÄM?£«0ïõÏ?̞áÀ"?Å鰃ýj?ཡÁ[T?ƅf•ÏúC?Ð5Kö<v˜?Âé:…{Ä5?Öþéƒ+?¶Ã¥×v'/?áHŽ‹ëÓp?¹-.©ý
3?½k""ûWØ?¤ßÜ£H]×?ά-4ìq?¬¨¶™¹âÖ?âÖ¾TR×W?µqŽk³ÅN?Åøú¶2?«[µ'Õ|Š?ÛÝ3­©ž?Ìí0Cƒ|?áOTݹo?Í=D?[EÝ?˜B)w
5?•nc?جDìï?ɧ.¤ûnî?܋wœt.?ƛ"!ڒ«?ÆùWû?ºð$«0ù?ãC»¤†]?¶	øô'lœ?Ô÷J`·?´JUDÈ4?²P¢Rý]? (O+@³?ړœBI]?«ËB²?à©>cy2?¬ëåò%¬?µ$Ešg}?—Ç|H(whMIXED3FGL J0102.8+5825@_B€®IÀ¨!ßβ*À7‹dBSbÀ:ú3ºA¯Î?ú‡Çßþù@;ºjŸ†@²,±¹Ëé¿ÝƬ_¢…"¿ãÔ"‰Sw¿åЭh>¾é¿æÙ¾«T‹AGNfsrq?ï•/|ê?…á›!?Q
?Z÷Lbd:F?[S[Еï?‡U7ržÒ?"Š£;ì°¼?îÄÆ\à?½‹Þ´ÅˆÐ?°™F'Λ?'K+àI%?«2_f‹Þ?»L|ðÁs¨?ìÉg"
?¤\-¸¶?¦¯yb"
>?™4a—°Ço?¬º´ÿõ?žèÿ
÷$Æ?ïë=Œí'¥?oý"#d?!e?"yhñ?Cz®¿Ûc?c¬Þê¿þ?nÕhaFL?ïÎÉV˜
?‡ÂeÝØÍ?ZQÏ+§ó¬?je"¡['?r]§§V¢?Õ>Ë?ïs29¥Î?øÁÚ
Ú?h×ˎa}?rœS(`7H?Œý~æýßñ?šÛF?Ýï?î"kèäãø?žÇzŸÐ·µ?©oŸ[?"@É`ìõ?žšÙv¯–?–87Œ"Š?ïüØ-ª?D²€á'º‰?ðâÅÖì?>§°š6?8 ÷_«V?CtxsF5AGN3FGL J0103.4+5336@_/0¾
í)À"mµ'm,À9š<Z#bÀ;•µav<¿õr`''èu@®µ©D²@Oë L'(¿à…Œ¿âõ¬¸}¿ßµë–³Ø'¿Ô=ڟ%þAGNbll?ïh37º×W?ˆëC8¥?`Îê"ÓÄÐ?YÊŸ:×]?ß»ÀI¬}?‡,ýÄEÛ?îgév"IY?­š%½:?''*ÌgcE?Œ¤iƒÁQ?¤÷â§Ë#?©ŸPú?îQϸ[óé?'¦4¼Þ×?'Ñ×Ð@\­?øRj?¡z"Øa?‹?°'?ïMڌåx?"EZ0y?.>qiÞ'f?1üy1k<o?–1~‡'[?"%òÑ@ìY?ïÎër²Ù?nÒw&'ï?KUY&5£?CcîçP?u‹ßA¥"?l—‰Êõ¬G?bq÷?–Rêï³½Ã?f‰bÎÜ
‰?lgÔù½Š?‰9NºªÈ?"J"QDæñ?ïhî|'¡b?u'ÎW¾¼??Åaª‡+?hý{C×Àþ?†A~T¸¡Ä?kÎQՈNÃ?ïÜl÷+?_ƃ",ý?
Ó:)²Œ?'%Âô?q"UwTÅ?^ýÝÛÑÄ!AGN3FGL J0103.7+1323@_âx £
·ÀH¯8à^*À:-m\ú¬ÚÀ;ËVN?ì~fº–Œ@º"kì­?ÿ½'ÓY¿èGr°K¸?––á"–5È¿×Q\`uƒ¿è?iÔÉúAGNbcu?ïåÀ"«?cåÒµžk?]µßrØ?]F{£³"«?X* ''S°?R^…©¿?í™äƒ³å[?©zr5GLª?•ª¬ì{¢?'Ó¡« }?«Õâo'Sw?¤°¯Ý>9@?îB½em{?˜ÈG|ÍMT?˜»èИÇ'?Œ7¼xÏq-?žìjŽù‰m?*óz‰Ô˜?ìfo†SI\?¦~B ñ?ªE'{"÷?œìr\þX—?¯Su'RS?žKŒ¢8š=?ïòæ܏ÚË?QÂóe?J¶ä†×ØW?G%˜•}?I­¨L>aÚ?CAMa>\…?ï=U¸1¼?ˆ9z$G?Uu¡Æz?{eT×i|$?UYUpp?†dÙùz³?ï>F@oöw?‡Áî.‹?ˆfšsF&?}ÏÁâ«Ú?ˆÕjä.?zÙ¬‰Šq?î}ûzN£?‹£ÚD—z)? [k×+°?ÝÕð¡6?'ÙáþÐ:?~RnØ¿æAGN3FGL J0105.1-2415@eZ`˜ÀUréÅ+À9jÑáÃôÀ;Üó…ô¡?뀾iW@@(4'@Ý砍©¡¿åË,AZ¿è'þO{¾<¿èåx.(Ì¿èΆ¢éE÷AGNfsrq?ï÷&
¼ØŸ?KàØÏ7ÖÉ?:Ú¯gÙ¯?8àÊêß?FZh–ܲ+?C¤Õ¸SN?î؜K*z?¤/ՍiL?lôÆv&?‰98}Ak¨?9oT¥? Ý±IÚ+¿?îLjõŽ¯?Ÿ-½ÿf?Ša;ØhúO?w¦yÏö?¤§JY°ïx?µ'vIÍ?íV§Ò¶?¨cf¥Ó(?"ÛNîñ'?‹©žÿœô;?°í²En?¥z!ÀUVZ?ïúÎ	㮑?>?6µ‰¥?2nÚ¸oÙ?,ÍÏ2·Òç?7‹AÚ¾'¿?3nl¸éÏã?ïgª3ÎAJ? ½Ñ×Ó°?pbŸð;_ÿ?|§Àn/¶?ä#Á™'?j܈OÆò?ïof®ún?˜úê:Û?{ëÜi›L¿?f®+•8Ŝ?•×'5?—îܦvP?ïg‰v¿X?ˆÒ.ò"ý?€°'®£?j•ð…Ï8h?†0­—´Yg?…EÎÔ)‡AGN3FGL J0105.3+3928@_va€M˜9À7R_>SùÀ9î㾀ٯÀ;Þ
,8m/?Ó,×(ñ:ë@¼e$@›|ßy¢®¿æO¶{ý|m¿ç´2°	%K¿Úµ†HÂb¿ì@÷33™AGNbll?ïå‡<ä{¯?d"Fa
?V²AXÚb?Vƒ·!?^?Es¨Gu?[lò™%†?î¦Äçiõ×?¡˜EÉ|¥?ˆ«1xqKŠ?…‡'mñÄ*?žÑÊQa5i?žc4n ãÞ?î€Ëtˆ3?'\ºi?— ÿ¼Ô«??ˆ>èîÍoã?˜Å'µ˜ªf?‡KíE;"?î"Ølh3?•üÚÅfÒ?Ý¯i€ÊZ?{uȆÒy­?¢;
_H–Æ?"ʋP—?ïòÁÆx9?R˜7ÓÛ¦±?JÅ£­i?D€SIøR/?LÇö)W×k?IDöSº¶?ï}ÐL«v³?ˆÆµÇÒ°õ?rôÊO-û?k"á^ŒJÏ?‡‡Ã¬ˆL?"ÊQÍqF?ïTÔá¡Î¥?ƒG¥©n?‰zÝу ?~}ÊG—²N?P³ÅÁu?q¥Iˆ"¨W?ï¢jeÏg²?vË
[Ÿ?r&AN|)d?]"Uݹ v?|¤‹Ë/Õº?sÓRŒçAGN3FGL J0106.5+4855@_^́'²ÌÀ+¾øßzN{À8®=Ç᫁À;Sà0Vßá@Úi=DY@
֛©"8‡?÷T™"öÊL?èÃQ¿Ù(…ÈßàÙ¿áêe¿ïá¼hÚ·PSRPSR?€¸DLY£¡?Ž-ŠólÞ?îk)H«h?¬sùuù?¥Znx"?© )e«¶?w¢Mg§Ý?ª +êÇ?í'…æˆ?¸Zc:"Wµ?µI«÷Öjú?´µ€»2b×?¡z¬,½ª?"™ú5½[~?룡'¤q~?ª:¢1Q?º%*j.>?¦ÖËüˆËB?{»0nçý?'=ê£Ï¶ã?í"ð4?¦ÆŽà§ ö?°0qÅ9`?¤#k9ëÑM?i.³6@¶V?wÅXýƒ·"?îÁÃU
û?«å²çu?¢Pß~pÂb?ªñ¹h²j"?v´Áö×x§?†´*ž+?í(Òûî?³j¨¹[?µT•FûFp?²½Q÷c?©øÔÿ«"C?›"acN,?ëY;¤µ›G?§æhñ"\ß?¸9¸Z}c©?£Áw'UŽ»?žG4Óäq™?‰.؉B†?í¬¸ìVf$?Ÿ…'¯tÁ?¦ÖЧdî?™j>[\&"PSR3FGL J0107.0-1208@a.T2TçÀR¤• Õ`À:l,µÿ+À;äkŽÄS'¿¢—z\Få³@åN`¶#=@qŸš´¿æK£ê«Z¿à>'$e™¿ÝVÎ:WŒ¿ê±K}"÷AGNbcu?ïŠW¿¯'å?‡‰ã­Q?§ÓJª?"
eÞ?wÐÐjûœO?t` è7c?î>tz®Ðk?©þøÇf+d?' ÕòíB?ã}·g•#?£M[œk®?Ÿ&˜<™±?ìõ©š,»?žÇhÕn–h?§VU‰4̯?"Y/ÔÖqì?©OØlœ?"¡‡ñóÅ,?ë÷÷ÛÉ?¨'ªèí?—²#…›U?Œ	ÉA!êS?½‹·a^Gg?¦à¸…û©š?ïÖü«Y,?k3÷‰ÿê§?fōþèÍ?a"^w*>?b=Ç´P©b?\'`)i?o,ø?‰Ü¹ó¼R?tù`ßWt?z<f_ÛÜ?ƒ‹\|D*?b¼ýeµ«?î·[é¡?ŽÈ?Ïï?–ˆ{]E4Ð?‡<T墖?'Œý¥É?|åî·Æ_?îµÇ³ÄyR?‰Zì¦*"s?†Ý©¥7?r=^›CûF?Ø4þÈ?…o=A‰AGN3FGL J0108.5-0035@`Ž2ßP]ÀO"!ÀD(NÀ:_-p{"À;ÍaÐÕp	?ç*Î$20Ì@$È´º1@&H «L¿à3×m5¿âÆïD4Ò	¿êÃPċ¿ïÿLˆ¼ AGNfsrq?í':7çÖq?®wl1ÒA?®2ž¥N?¬"BèäI?'t³Åº•Û?Œ¾ÂwÓ.?ê>à²Õ!?Àöûg{¯?´¡Þ¥Q?³°—
hѵ?»4*Tz&?´fm~Û¬?êpåáâ"?§@Å`$‹ƒ?»¿uK?£,Ì«ƒ•»?°¹Ë…y?•Lv'p?ãZ¡üÖ?´½úE,º0?ÍðÆôyB?´1Ž¤ÓF?Ä¥då.[?­sOOjï?ï!:w˸?•@ð‹ö—?"8¡…ký9?'rÒUXê*?@÷¡"?z±ê5wâä?í×í²þøø?§÷ýåå?¡<©ô?ëÍ{Åßx?¡mèB¢{?–/£Õ´\P?ínÜ=¥t?—À%8b‹Õ?«&dKa±?""ƒ›… ÷?œ—ª$?ƒ4À˜3WŽ?ë¶ÊVûº?¡ÁÛ
I˜?º.ÓõW|á?›˜yr­}™?ªÖëoc›?"'7ÂÂCAGN3FGL J0108.7+0134@`{Ãá`xÀN	@¢CÀ7yÚh–ÂOÀ;Ù}µ7…?øn$Ù(OÕ@kä)µ°ü@Ÿå]½Jy¿â ÞÀŒš¿æ¶­ôøîq¿åe³™ÜÚ¿ê+\üŸBAGNfsrq?ïå'ÓóK€?aìü4qá??aÃ7È¼E?^úsèqÑN?R)胤÷.?JW$hQRê?ï˜Ó4Há?ˆÜø­ñ?d:$‰bAü?iXHle
?"¼©Ü5_-?"•ÜÁN£Ù?îK;ük²?šăh…?žæ(«Q?"6¢rhú¬?—²WÚÐÐ?y
ÉUÌ?ï\(¹¡e°?"SMg¹c?XŠ¯ÄoÛV?cö &Ý?'ò=Ó'ãQ?'ã۝?ïëh±ø¾¡?c®sŒ'ã¶?`+×+ô†?a²Ù^¾æ?A­Ü,%&¥?;ñ›Ü^ó?ïÕŸ§Ó?p¡þŒ÷@‡?U¿€Œ~'?UÑ,u"\‹?pkò%þ–?i*Ô>¯ó?îÙt]}'?"­hÜÌïé?—¦g¿I/?.³RÅx.?Šlpíu[?'(ë¶à?ïÚH^Ϫ^?t.š–ûú?OœDo—ôë?Y0"ñ7?mА3èÝs?rIjÞïYØAGN3FGL J0109.1+1816@`çßã*ÀF3=?üoRÀ9ÌjNRsjÀ;¸a†,ÕK¿â@2,…Ú@
§Ü"@k@Q–ߪõâ¿âÇ6cݿׯÛ[A*~¿âðÄQOû¿ÓÔèÍçÝ}AGNbll?îm/ŠKÜ?±°fË_;.?hׇͨ‹Y?p6N
"™?§ ,Ѐ|
?±s«ÛPù6?ïWêkTs?—ú
Á—a?n°è€pÌ?x¥—}'	?',¯xŒC?"1rY\êF?ìã=Šq€?¡ØM<&y?–HÆ{ò•?†3òïÍã
?³P䌩^? 1s8³…?îT:Ô+)¾?›W<¾&Š¼?bq*Õ¸¤?dD,ÜØ4Á?©•@¿¥Z?šÊ+R;±?ï"(•ÇP?"nÛç>Z?R®˜w7Fw?W£&"ÔL?ˆàŸÙ+?"¼IFðÕ@?ïÏÉkeÌ?r]³
k*Q?UKÈ#ôg£?QïQ8¯,?rÈX[z;é?oã*WzŽß?îê _?'
Ϝò"?‹éK	s?…l†xðü?šGYÇ Ú?Œ¡ußg?ï¥rãàï?tâí'k…?B]µš[?7‡iýÖ?…}kïF?s¸½Ø‡zçAGN3FGL J0109.8+6132@_H?Ffí¿óååÀ
̜À7³Ä UàÝÀ;TáÙ¤?ûÊÉĕF@µ|Ï'@'X³ö<2¿ãáÕRàÖ"¿ç?ÄEa*Š¿ëö•¿è¯ürŠi®AGNfsrq?ïD÷–)^?›Ô®ÞôCi?ë œn?˜ê˜QÕf£?}Ä)Šœâ?|w?å»Ù?âV?»ìo?Ø›2!™?¥ú[ÇÄ'Ì?±(Z®ã‡î?ؔ6Kt%I?Ö°—ŽÙ¾?ìÙÅ0v?w?¡{•Ã8]ñ?¦½Ô²*|Y?—^] ƒ"?«¥ØCÝ×4?™[,e¦}?ï撁UÍ?quËéÎ6?5k!Îmi?IÅM-•)!?fÀ–˜?p™"ƯĂ?ï†Xpü¹Ç?±³ª-Ñϊ?ˆùŸªï?±µ~Çf?eÁ~ñÙ<?h¡ê)ÌÕ?ê^<XBX·?ÑíVøπ?'ùƃq4?ž2rÃí?ÄGÕÌШ¤?Ðq¹C‹£•?íš†©°q? º	Glm?¤Eè߂?–˜V̶²?¢DòzÎp?•˜UÙ=ƒ?ïùS{Û¡/?WA9f—#t?%­à7y?<Ç|P?EF™‹™eô?UO%MÊ=AGN3FGL J0109.9-4020@qÿ4?¢­?ÀS¿ä†þÀ:]Y#‡Ä…À;ÇOr.Å¿ÿô
]ᇚ@
~	æ]Â~?û£l`üD4¿îë]£–"ú?ï¾âá-¤J¿æÏÊ|ª9i¿ÉX­*ÅüNAGNbll?ïÈ
ãöèˆ?w˜÷V¼æØ?D`·bÈÆ/?Dq<[ݺì?yl÷ q³K?vÇáªy@¬?ï™ä5Û?h?ðÅÇÂC?c-•}=ã?rRÆÚÆ?"ŧ!i©?‰PÓð&?îDï²³z?'|‰Ïæ?'×ÓEtÄÇ?€A{kÔ5?¢Ò7d®ÿ?‹»£ÇªTü?ï¬:â?†äk¡zà?J¶L¦?qhZÜ"¹?ƒQÏy§@?"̦ÛMMy?ïí(ô"»€?`J;"ðä½?2Wç{	J†?2dÁÇ@Î?`Œª‰t<?]À *$?ïሻÐÑ?k'HÒر?L㛗U&Ý?O(Ö¥}Ú&?g>]½T?esÑ{å«ú?ï1OðЄŠ?' ¹nƒ8Ø?†Ä
goñm?{Oï¾S·1?Œçör-\?tݺ på{?ïî\éÝKB?`Ιnd+>ôÄ3(êU?PX&Sã8?ayèý•?`"ÐmðæAGN3FGL J0110.2+6806@_,‰a=1º@;N¿«§
À8´¿%DÀ;´öí1Ç¿ñÒف;)@Æp÷cú?ÿڑÿFq©¿Þª¯ iú¿âq«h#*¿ßíž
¿Öì,39¾=AGNbll?íÄ@³ðn?¨Í%	Áù?ƒ÷!uÍ·Û?{ÎÞ¬?®¾7†õ•'?§zÆõ÷?é'Ùù}|O?Ï_"++ãð?šÑ¥Æšü?¢åéÖØEO?ÆZu¤>Z¦?Ìr d³~?ê¶
'Ô¹?ª¯%6²L?¦#›UOu†?"qåz·Žõ?¿=Ú‡'ö?¦G±8tì?ê¦c*%ª?´4»eʞÅ?kBž¨O?qEÀ5³Ù?ÄùiKP¾è?´ô|‰Öh?ïA'X¾™??"F®~ò¾?p¸
&ú?kø")¨?"ŸÔ©â}h?'Cømނ?î±ÞcXY?±Ÿ¿d¹¥ï?~rÇÖÂg?ŠJha›Ùî? òPM¡þ«?­Ð\("Õ²?íåuqcè?˜åÿ"Cp"?—卟 ¨R?ˆ,6uÐ??¥µèYmZ?'mx°>Aq?îW—Ë'?–C¼©zH'?Juõ°d¡É?D	t"‰D?ª«tqó·?–"^û·<AGN3FGL J0110.9-1254@a¶êá‹ÀRÄqýÌIÀ:pµÈ¤I À;Ó	¹½&¿ìÒÏbJÅC@ȍ¸dàÕ?þÍÉ¿|,K?Ú#pqpõO¿ÚÁÜÚ$¿ê30ïꑷ?ÊY1y´™AGNbll?ï·:燎)?€
«˜?m[{F2lv?q,>˜[Fô?u´Î0¹*?xUs"' ?ï–ËA˜Œå?‰U;8Օ?cÛ&Ö?sa4³ü?…\HÁ"ÿ9?ƒÐ®@-?í>Äê]à?š6ió¤?¡,j.V†s?ÃZ—­¤?¦¿©ƒ›?'£ïðë<?î"Oa¤?¢?˜ÏÍ»¾?F ¤)†\^?\ÊÅ­"
l?¦fx{"L?¢/õmÙ6
?ïãVçöÒb?k:íM)K?Rîa¼ò[?]_Ô¹ÂÓ?c§ ¾2‹?cå/:áª?ïÞÿ!ç9?kÖòr{?PÇÀZböê?T]/=?hœýÝ×P?cÝ"vG¾?îË.ßC6?"ü°¥?"«òùœ?…AjûÃÒ ?'îJµ?€M½Oç«ï?ïÄÃɘåÀ?t']c*Ž?Ñ?ã.ä?Z/vØ«?}VÖöÑ>?t|ŠjÖ¦SAGN3FGL J0111.5+0535@`ƒ'ßüTzÀLvÆÀCQŽÀ:"#bۗkÀ;áž*øÒ¿Ï@h¡DB@»»+9¿"?þ«®>Â2•?츝ü]fÁ¿ÙqÃÇj=¿ËåòFÈ«¿â(4æezAGNbll?ïøt 2\k?CþßYË?"ùW¥:ï?%Шè?Io9ӭŒ?A{EèXþ?ïŠQçö–A?ˆâPÐN¢Õ?g‰ Xò«Ë?p³c
Ž"?‡‰=é¶
À?"ûݤ/]?îþð|ïÆ?…rj2¥y?‡ž5«J«|?tϑ£
–?"RՑ¡»m?
Àé,êp?îáCC÷{¢?– BÐì€?T­…aŽÈS?TMÎÈæ¸?¡F_"lŸ?–JSí/FS?ïú¬·Œ&r?<;ž¢°áí?æ¹k+cÂ?û€om^?BK…S¾ä?:™¸MðÇ?ïØ섑ä]?p{´ã>V¼?SœˆÙý:¿?SAâ@"?mE76¶í?j]MzÍH?ïy±Ãm8Ï?v֘–¤ó›?~o`2K?núW§P‡?''×t˜È¬?kÈ¿ÿ	b?ïÃåõ·O?pøvê?Þ?Hfà.]qY?:5ìœQLJ?{)cƒ4Œ?p81îdJ AGN3FGL J0112.1+2245@`$›«–òÀCîŸóOîÀ7FëÝ3L^À:£!
;Ã%?ø>§UCÿ3@Å~öU1?ýøã
Hٿ؜t/ó¿àäJ\Å}οáC€»Û¿ã´¼~å§ÿAGNBLL?ïôy¥™"K?RÁqêF?,âûÈ'{?-XÉã|?SpUº\ß?Q0õˆÞ+‰?ïˆüï»us?‰ån­}iG?h`@æÚ©?s‰ª‰¼ö?‡¨³Òz±?ƒ*A
?í|Džëh? '¦׈ê?œ–ñÚÂA?'­,†?©ê³-7[?šÃÉëž6?î×pH<ð?šmy´B?UБc¦SÍ?h0í-­W?¡ÚvîØÜ?šªà"pì?ïûáÓB?:½Ó(óÿG?"Ã)'¶r?!}ËÊ£M?7넝ª1Ò?6¾kßv£J?ïÕé¼ϔ?o¤ÁУP½?Uÿ,$‡?SáÎh
±Ü?o®EBE?h£[Œˆ,?î|ÛÇ!ÎB?šB0¬9<3?"oB»¸é›?ŽÃ:ñ¦?›õDaÅ?'Ñ|)´=ç?ï  Y¯ÒI?€"¬ÄŸyÔ?SÁ®€½?P7ŽzjI?…vQnqG¢?€Nyû»˜AGN3FGL J0112.8+3207@`)?)
»À>†§ ÃY‡À7ùpQ¡³DÀ;]*Ãøèµ?ç Ü ›×@räOOt@æšà@œþ¿ã|Tò+¿å{{°iX£¿æŽ;@Œ¦Ü¿å±ÿaýÿAGNfsrq?ï÷óÜRž*?E;ß/&?3Óõ0•?.¦zí£¯?FGuª!N?AgþYË?ï›V§EmŒ?ƒ	— ö{6?cÌ»>ãË+?dòÐZZ?"7'P%X;?¸'ðÍ&?î¿ÌÜg?'8YLrUz?Œ{¤½ÄY&?f¸:€nÏ?™È'7¿?‹ãí©$÷½?ïñŠ;$:¿?eßzæ±>ü"—Hœ×?;éðÚÑ?\y;3ìnc?eÔØóbÿ?ïüè	­í}?/	EO¿|?"JGÛkh?é—j†?/cHè¹Ï?%$Þ\p\?ïÛƈm«?jA4ˆ\Ø6?R#?5M&h?PCQD½:c?kә抩ã?d4ðVU?ïlmX*Â?'×i†ÿ'?}AÛß
½ë?uÝuYdõ?†C®B­€€?|Þéus h?ïþ+$ö…?;úgï6[í>烬
q_ª>öÁ¤M[õ?+ÎÔžàV?;Ξ"6Š·AGN3FGL J0113.0-3554@qJ@WÀTLŸëÃ2À: W À<¾ne8i¿êøü^=@´½uÁÎ@ÈŠ>ˆ¿äGÃ*.C¿äódfº|Ç¿ïv­×û:Z?åeä J…,AGNfsrq?ïûÆ&c§?DqtC݋?v‰AÅ\u?Ԟ½Leö?;±.….;?B[I7˜XÀ?ï©2¯»Ö?‡ørEdP?_ËΠ£¢?eÓ׊@?¹ÚC8R?" žØ×?î¹d;؍?"&ƒ?‹Õ0Mđ¼?€ÉeߌÓÈ?šèàf£O?ŠG~¦½Þ?ïï"û°m¤?hÚÔ¢:É>â´H)BÌ>ý©f¸áh?`hèz"÷?hÛ A§áÏ?ïþ
·5ƒ<?8Ð,ñ·	??	â3E?¿îw¯á?)DÇÆ<qP?4¬xéHð3?ïäyîՆ?hÅÆ>¯ex?Kƅ'Rî¯?O҈OŽ?d"pEPÏ?b='"™üš?ï`§á—u?ƒúݬ‹R?~´—k%ò?uM͓ž9[?ˆÕ-T³Ý?€‡ðÿ´¼?ïþ"
¹Q?8F6Yb°>¯µàa'¥E>Íç…Ížÿ?&¯kð?8?/~AGN3FGL J0113.4+4948@_¥>¢ŒÀ)Í*Ž:ÁÀ9I݂&¶MÀ;ŒÚF2y?–ªnxåŒ:@æì·£ÅÂ@dŽÀ!ß¿ã¦oÓ¢~ð¿æeí;›ü9¿ââëYͿ൮#O¡AGNfsrq?ïÔوòØO?péʄT*R?]¢Éõ~0*?X®xG?%?lUԏ¡
?j£JJŽˆ?î-¿GlêÔ?µª¼A§NÀ?­ód/7?•î?›óÒO?¥¸Êô?±ëÿ½ð?íë³jæ?—ÔËíÖg?™L£¡Ï*ó?…Rc+Ø;?¤ž}6À+?: °|C¤?ì·xX<"??¡ž¤Ã?…ø>hçN?~¡§í=^?·…5s$Eø? ùÅá©â?ïðˆÖ4'?WŽýmА?F»=ñ6ÀZ?Eè!ÈÞ4P?S'Y{÷¾,?PâZö'?ïf­RÖ^?›Š6lj¹I?u397[B?€œ|…5ˆ?‹»¢Î
Ï?•zÑ~ùŠd?ïO䬒o¯?|rNòñjŒ?ƒmÑG»jw?q5öÉ­Ù?ˆ™¡¿Ç?q3A4ûwÂ?ï9{ù9?`˜|%ÿ?p¦;[}V¦?XêÃfŸW?"¦òh?€•a«µˆµAGN3FGL J0114.8+1326@`tÿ´€¦ÀH…>ÏuÀ8õ¾smµæÀ;oU"‡"¿ü¸0ÆFuÛ@wFwÉM@žL?ž¦t¿×dÄ9Lʿ怲u¾æ¿Ýe­›{"l¿ØtiD£YGAGNbll?ïûÝz³¿$?:•="(Ï?
–Í??%[ºQD¹?=ÁPg_?8Ïy^Á·?ï—ib¼…#?‰ø²ÞØö£?f'!ªšÆ?zò)ƒ×ƒ?"›ßÕ(ƒ?€Ý'¯'ž?ï*M†ú
U?…½Ê¡Ê!?€Fi"ʝÒ?rðÊÄ9g?'"XÙ¦s?'bÝ¢_tZ?ïÁ]}(;?yÚ¥Þ
‰´>ëqõcæ*>ú% µ§úâ?C¾e¿Ä?yԚ›ª‰?ïþC[Ž4û?#¨âê6T??ñGF?/šQÇâ?&:vÔh0?!!~È~?ïޞ8N?k"žê²­?P C½Q'8?Pݵ¦3;²?i¥ßð
€?d—ARHá?ïšE Yc?vq¨Gê?t­+2¿?fdR˹Y?~Þ°7sß?qU³•ã?ïóûÀ³Âm?OÐX[í`>Åy…­Iš>ǁÿÚk©á?Wýö#Öôl?OÏOéß©AGN3FGL J0115.7+0356@`Ѿ ºKÀM0¶ßû}ºÀ9	ÓöeÀ;xÃkúúÞ?³©ûæ"°Å@[Î\ïÅ@ñÌ )–&¿ÙÊ.Ýc¿æ€=Ÿj5¿Û°üýl&ð¿âþ3¼×?AGNbll?ï»Ð¶;eÝ?…ßÜó+Hh?SêeKd?R®Ç["U_?}Oê2•&ä?"Õã_íC?ï(äà-Á?;ë"§?y³#œþš?ˆTYsٜ?"'z¢zÂ(?•©pòÉp(?íϞ±0?œæ·Qû?"â‰Vé6^?ƒÁ-ήŒ?¨"Ð=6ð—?—ÿ¦o¿ T?ë"Z\Ô?ªc4'â¹?}…ɝã>J?u-oN•W÷?µÀIdUž?ªÁëݼ?ïí(èµP?mõl¤©"??ö<¢LG?B®
ÀU¨?]°ŸW,/?j‡R©J¯?ï¿ü¤.&?MCL×YN?`Iå}N¡?`HÄ¡?wÜÿÏÏ;?z>æ1Ý$?ï6.@ÁLw?…Ap³}b°?ƒ¨ÛvÔ?u'$Åö‡?ŽËïñÙ»b?€«XjC¥z?î¢Øhü»?Œ°c4­±ª?ouüIÿµÓ?[RXE\?£Ûªk»õ?Œ#®­h^AGN3FGL J0115.8+2519@`;[ߏG0ÀB›dÜY2À9ç
¶<À;aìNrSÚ?á«ÊžŸ=@Ù»$Ù©)?ÿÊW!O!¿åޛâi¿às݅+Îe¿ß>ß)×Ðó¿ÔkêÒÏνAGNbll?ïòüe'g?P¼ó–DÖ?:Ÿy§'$?54A4õæÊ?S_Wqœ¼?Jï9©g$?ïl'Á3¤?Ž4çm€ï¦?jzےHh?j]ècº8B?Ž<ØÉ;e	?‹‡eÐÄr?ï!·Rg+?…z;BfÑ?"ÎMUsO?uå+D§¦Ú?'a›?R_ÊF/?í¬î');?šM.·á?qËó;R
?q"Û2»?±‹"ÍãßI?™å †²\?ïù'yP	>?=˽Ɍ-h?1Þ.-¹é•?1m:z'»f?@ÇsÍ$?3€êðd?ïË1ûrÕ?täŸÍËZs?YÔj}²À?TN,0Ô?t
lf8ü?ržñ S`'?麟F--?ml	ˆ%é?rS–auÆ?^'¢¯€?yÒçÁÝq?fÛªf–?ï^³®åþn?{_æ£w9?eÌ£Îþ´?VP‡6R'î?'oõ¨°…;?y"4QN"äAGN3FGL J0116.0-1134@btÀœ<âÀRZ?ßéàÀ8ê`ão¦À;¬\ê½?êë5·¶©å@®!èÝúr@ÀPÀ6çH¿Þ.ëlcð¿ç´Ak	¿æ¡g"âöZ¿èRàÄjAAGNfsrq?ïúÃÙÅ>õ?9©Gñ)?0ÐK
H:?,R@Dh—z?9åVÁj'?2\ŠÁ­ã?ïžLÈ@Ý&?‹d¯ƒ²K?cUœ­]æL?{š³ÐrØ?ƒ—f¸jš÷?'yñÏ`Þç?î™Õ Xe?'àù‹ŽíX?'v:ƒ"er?ƒR¤£rY?›hJØpê?
ä ý0Û?ïÞt]'«ô?t¢ÚðWê˜?eH+Ê"?.‰¢L‡?pL<7ùt€?ts±·úV?ïü±›Ã.?1+'úžå.?&ññ3»{?!]gïË#?-ý;'"w?*9ä2ÖJ?ïà«æ<#a?k;ÈÒp?Në+kkê?Pél•ªw?g™Tødß?dñØñ‡\?î¤ZÂnO?›¹tå¶üÍ?ƒëVëFz?~ÐÔUA¤à? Äµ>JDp?›kt"½Áá?ïûLK ÿn?K~ô%?¸]äñÖ.?˜ò°ØI?AN=u{Ð?J␌</)AGN3FGL J0116.2-2744@k–PÉSœÀUM`#UÀ:jâÌéRÀ;ñ[dR?¡ZT¤
ûu@
—&`çÌX@.ÿ—ÐA?éÄ×Ä]Σ¿ÞɌráì;¿äƒT¸þL¿Ó¦ýÇãÑCAGNbcu?ïÑ{r½å?w'cèXS´?Hq×­&Ï?E…ÕŽd~"?t4%·w¸?v¢¦éÒVÐ?ïw@Ðn†µ?"²¼EˆN?q¦ƒ¬,LD?…Ó…,A€?‰\Š
˜@"?Š'pÊ%O0?îJÇOˆ?'öáùMÁü?"'?pîT?[Þ5óJ?¡ŠkUòV?Óþ˜—~?íÌ<*õïR?¥O\u×¥?qjÞ©ñ»ý?rñåºÌEœ?°‡p¼Êƒï?¤Ýš^b'?ïêÉ[—ð?hþÐøßû?9dãSš?;t¬B3µ?bWíi/Ý?g,3sÏ¢l?ïÏ~j¿¢?|sPŽö˜ò?V<}o¦†?[ìë´B4&?rœûum¨?y0*ÞY Þ?ï2n2YŒ?…мgò$?…tx8P†?tÿµ±?ïûEÉp?£QJjÈN?¹³ä?}²<Mš.î?U‰hzŽûª?Nùf¡v­?†©ä´WÝx?|V¯VpAGN3FGL J0116.3-6153@rœû`(^ÄÀK~'Éä»À:ѵiÙ¸À;å€~?¡¿©M -Ì@¹"x˜B,?ÿd¿9Ú¿ÝCbB"#¿ådá¸['¿áuÎw¶‰®?"%µy҇AGNbll?ïó‡ÐY?SGÞëý!{?$PÂÑ
7?!htÑ|[@?WDØ}¬<'?QÕ@É$ÊÛ?"3pg?…S›m
BÅ?c"škr(?fjF	čÛ?…´£ž×?'Uċ•_?î÷¹S·üË?"rÄi?†§ë3Ú?r~$œº/?•ûÆ26±?~~きgì?ï\Ng
¢¢?Œ•YîÞÅs?7®ãnÙf?EËðéÓ>?"wt—?ŒS"0¢U?ïû/>dA?9~_BHŸ?ÌÜ9hJ«?(Þt_?@‰j3Îhß?6â	²—øÁ?ïÞ×ïÉ.»?iq
2k1?P¸6
ÀIg?QÄ¯CS?hËõGNwú?c+7Ž|"?ï'Ê{Ÿï°?lƒM̗jç?uŗ3@ÔÆ?a é¸ù'Ï?€j•Ùçy?c44nSf ?ïçã|øµD?b݇õú?"ôdô w?&Ä=&€|?fí<ŠÉï?axcÑÒ_AGN3FGL J0117.8-2113@e:Œ¿+#šÀTdŽà3·À9Is§—‰À;>e§#ÅØ?æj³Æ§ªæ@Ÿæ:@"Áÿê0‹?ÈÞ÷5šÛ¿çpws¡YÏ¿ã¥yéï¿çKÓ µ'AGNfsrq?ïóŸ¥'
?S^ÑÀw?InX¶ùÑB?IÄ7ìÎý3?Jo)2MÛ?G¹dAŠo?ïGW™ˆ'?–Ö—ÑÃV¬?vÀ†ß×è?"€ðEc?'"¯¨WU/?'4:td
Ã?î›þ¦í×?«˜´<><?'T7ÈjÓ¹?ƒÔs8t¤6?š+óVõl?‡ò¾"ý®¬?ècD(V"é?²#ùúoú?í<Ւˆ?…@3øÿ%?ÌUGÛ
þ?±ùk–oü9?ïùWgEž?B"R2ŽIR?;~ðƒ¡&D?8Gö52~[?9ÅÖôÐðF?4A¬[9ª­?ï¶z0P]n?Ô¡mӌ?fÔ¤ÇÉýj?qøŸÈä‰"?yX•_N¢V?wÓ*ƒÕ?ïd§hŠE?'ˆ?Y?´ÜKàö?wãɖ¨¡?…Âq
»'Ô?| -Ép-±?íDÎé)?–ÖÕTÔÅI?ŒA¥¯ƒì?s+a«Š=¡?²W¤æ*¡&?–œñ³AGN3FGL J0118.8-2142@e¬Ø'tÀTorßñl¿À8HK"bаÀ;ô3C#k?ûÿaw>Oò@½ßtWj@š*ôw¿â¾¯CAk¿ä֛:…¿äá§fz¢!¿éþœJwÈAGNfsrq?ïtv
¸¬?€ÑŸåü?s i°ˆt‰?wõ˜&¹Õ?‰HŠð±?Œ'ìý§´?ïClϔ°Ú?Ÿnú³*ˆ?n	« ˜:?~
ð»hÈ(?"Ñ0²ðð¨?Ïùrµ9?ë71e[W?­#Ëîø¾?´ôE;zRÍ?£7 Ç‰Œž?±R/™ªôP?£Ñ)kP?íyB"Y?ª%´k=K÷?|©{Z²‡¶?}øš
û­?²kS°ã)‰?©‰Ÿ
"Áí?ïØ	‹õ1?qù$r?b†É6+|?ec4ñ
?eo«®¡íì?fe
³Ù¡?ï²Çc½zÛ?…ÞýùUñî?`ãò­ÚâÆ?`6Ö5>@Ò?~*Tۃ,È?ƒ"ðÈÓi?ìRÄûi³?§È®Òjä?°Û÷"ôé?¡ö3¯w)í?©Á#6Àû?kàíÄ~?ï•¥CEû?Õpû¹Ëó?
½«Nð?r‡?5à5¯?–ÉÛëH™ê?ßâì-lAGN3FGL J0118.9-1457@cl O*àÀSt`$-À:Q¹  À;Ȭ¶¬Ï׿º[Ï@'âã@
]7Ÿ©~?ü"Ëÿrfz?ïŠeöÔÞ¿á†áÖÃ-¿ÞœÎ¤µ¤¿²8}4‰¢AGNbll?ïÛ(D§°?kn¼àr¨?;:M¾'µ?;SsXB˜?p¸8¯3µÀ?i×äB¶92?ï™RÍ_øA?Š»Ž4V`ï?fü½Ìòëÿ?|­aÅ;aÂ?ƒì<TXÃ?ƒ^Z½â?Žf×ó?‰ÑžÔÓÇ?ÁÛԒîú?x%`xlù€?žÊ`Nô$?"°¹š
Å»?îfÌ4Bõ?¢ð"Â.ÿ–?Q5pŸ¯C3?W¬8ÚñŒ?®/纔?¢Ìö|ïJî?ïò6~ö?V&'|þ"?'ѵ3(?#öV¶A÷´?Y
ãiªŒ?UHAÀÈ:?ïàD¿ô?jÀ\Î
?NÎæDD?O~Kºuñ?hhˆ}ÞW?d»l¿Ô;`?ï\°Ÿgj?x"k›ô+¥?óL!ón?mŠ3)âúN?ˆÚ2$»,Y?pÂó&ø<?輦¬În|?ymᑡD?<´´êð'?6èµ
d?…t/1-åå?x£(6žƒSAGN3FGL J0120.4-2700@j²¸`™ËÀTáþ@_ŠÀ7âW5ŒªÀ:ÙP·¨xZ?î¯Xº@-•'ÎÏ0?þ E?z>`¿ÛôxÜÏh!¿àI€4ߛ¿Ú>«<7¿Ýï²!r7øAGNbll?ïÀeÆXiy?| ½ÄÓ?XO*M?[e±Œ^Ûs?yÈéSPÂ?yæ׋ÔÌV?íׄê=ª?Ãb5OGÍ?†"ìõ	?œ ÔçÕ?´Nàš>m?Âu±‡÷ۙ?ë®Uû?«™"!uê•?žýª`g˜?n›»ž+n?ºÍåŒÈa?©'RÃ*é?ã¼èöùñô?¹7žÎàîÛ?¶¢«öo\?µðûâ?×zÃèD?¹&´ÛІý?ïâ^DŒˆ?yí.wzËy?Gòø
9]5?FhâyRÃo?g¤ýOŸn&?y×ޅ%S?î|§kœä°?·RC*w?9q0	)?'wÓ='¬?¤NYZ]pS?µ6mŽ†'—?헻îƒ*í?¢2õR€j?™SÅßN­Ù?'z£×'Ä?©Ú^%'EC?œ6쑓YÇ?éàb¿-?©Ÿ´mdÅ?"ƒœÏÆ1?'ŽÆ"5?Æ€2ÀG?©8Œ/×AGN3FGL J0121.7+5154@_ìÀ§¨À%_tÿ†]}À:›=އàÀ;—f=Kºé¿êz¸•)¿¹@
7¢wŽ¬×?ÿ¾Øà×EÍ¿éîÃà—´¿ÐåI=ê#þ¿Ò‡­rOº¿èƬªËúAGNbcu?ïn‹ßzW?'®œ¡f?l#R&q?tA~Ìúõ?TEŸ;?ŽÐ|L2²?íZª³PÞ?´,Œ•Á?'@Ո2>?fˆ
«³?°Útÿ¿
?±¸"›¶Te?î@Í:/ü?"[­CÓ;?'"-xi?‹f½C"?£+,}.ù?ŽhkqF?îZ~.aÆ?œkÕû©ß?qáÐ
J˓?oÉ=ÏÚûd?¬žî6?›@Þã‹ç?ïÏf7Êû?våÚæ-
?S/q†LÚ'?S:ôkvïi?sÁ.LÞ?tjgšËu?ï4<mͦ?œ¾@ÆÛc?uÕ«¤þ6…?vÎtbˆÌ?"^}•«?—õ~¶?ïRåV5—?x'®ˆ´?€ý´c°ç²?kqüé=zn?ŠI	Ñh|'?oÀ:#®Ì?ïx_îZÄ¥?yç¡Í5K"?Xç$šÃ_?Oÿ`¸ÀN?ŽËڃ>?yüOhiAGN3FGL J0122.8+3423@`Hüàü.ºÀ<€ÌC:À9ò¯ñʳÀ;x¢?Zˆã¿ð–G²œ@
]Œ©ÇG?÷Áˆ`Œ1Ò¿ä"ÉÑ¿áÔ÷p0áí?°DS½¨}É?²žçóUAGNbll?íþ³Î	t?±ZqÄ÷?FtŠÀNf?B
zG˜?¯ºðñ/=?±Uˆx?ï'Ç1yÂ?Š}@(¬J
?k)'vçŽ×?|èW2¼ùÅ?"´m'p-Ï?€ÃC9\G?íðï|?˜{èÁ|¼?"3ªz³Ÿ?"ãh
¾+5?§]Q°Eu?"ò¾ÞS†?ï‡0ˆ*}Ï?"×à>S(Å>ö8Êâ?´;éÎ;Ç?Ž(Áåõ'?"×jmX´Q?ïG^6IƦ?›SPފ|?8ûø°ô?6˲Qô?–°IZþ-Œ?›=ã¤}ï?ïÚz|óƌ?mÔÇrÛK?Rž»åok(?QGDøÓ®?l6%/>?gzÝçˆW*?ï$Ƽp?/›B8?†q€Ö4ª?'îX¬¢1"?'⦴Ò]š?†Ñ'æCº?ïåiw?[ˆ,8Ó>íƒ
í]@>ì֖m—	Î?jaNe
•?[[¦4iAGN3FGL J0123.7-2312@gMó`Iì³ÀTmŽõƒ¥À9¤†ü#»À;ž_7ûÿ?͈–'ôø¡@'@'m€?ÿÐ1€Ö(¿êIÒ¿U¿É|ö«mŽ¿á©}~ÛÓ¿à+aé©ýAGNbll?ïò)#v
	?R{±h"?@†e®žê?8ÛèpËS?Sjr~" ?ML¼ ú¦?ïUP=—T?""Ž™‰Ÿ?q‡µæ‰;?qënaì?'j§x0?¸ñjêCP?îïzQC??‡‡ÀùæӍ?ŠLwÆÃÅÓ?xnâj|£O?"ꃰ½çF?"G}6o?í'½k°Ó?¡¡Ð'Ý›Z?'î.íakx?}YÆÄÚg?´dNÄØ8p? ì]å")?ïúiàïCš?<:2¬ùá?."*;ƒ'µ?-X°c?=nãZï²h?3az)´g?ïʑ'sü?ví'ð­ÿ?Z†vX?_	:ÔKÎ?tçƒÁoé?rm¸K<Ê?ï'!©"/?q^oÌì'J?wžÑËÌ?a
"tl£?`(­ã?j8mÁù±?ï3IÐ,u?€ŠKY'ð»?n«îœß€û?Y«sûi16?•ÁNuv'8?0p$X
AGN3FGL J0125.2-0627@b6"_õIÀPô'@.Ä9À:6¼ÿÐ/XÀ;×ÓãAƒX?ñGFÐôÏ @SU=õ"@©Ë€qt?ïj6&<D¿åĬ…%Ë¿æÇùG^'¿çƒ¬þPRAGNbll?ï€Ã)¸ê?Œ–c‹?{êyÂÎñ?‡[µ
øÒ?Úéý
?uåO¥?á÷g'?¨'g©3?‹qE…'¨?˜Ú½6Ý|?ò!CgJ÷? A÷QŸ%?ëwÿÓµIM?«*÷çؗ?µÿ*åSMÒ?¥Ë6/Ç?¬¬úඃ?˜¨T™öß?è
¡n¥?·¢%‰pdi?´m4˜Bix?¦VW1ŒŒb?ÃÍY‰"ð?µ²Äˆ¼™Ò?ï°»fˈ?fy%­ÿ?u­2º}?uöTm.z?r#n85Q?sÅç>¶É©?ïq3€ØO?WÍ°ó4?yBuöL?}QÚÌíi‡?‡'~Œ1ƒ?†Æ;ñÅ@?îka=:?—ið÷ˆéò?£™+9ށ?'øw[½Q@?–1j$CÓ«?‡	\l‰ãf?í™×¢=×ý? }"úOFL?¥]*
Ö¾y?'ð93^ny?¡[Ï'¨¸?—¿‹¸ÞÂéAGN3FGL J0125.4-2548@i ½ ßÞøÀT''?àÀ À:Œn7ìÀ;ãKÊíñ?ä)ˆ[òð@pÀþãJh@	läÛ¿æÉ "ì¿Ö±yJÕÍc¿ãPÎúyƒ¿çBӃdçAGNbll?ïûÕ]ÿ(?9|±¥o E?%Û^ìet?'nøÚ–?;K ôÖ?6ëålse?ïKýÈòl?Çõ¤;Æñ?rMK²ºã¥?pçôD,Ï?'ìôf'?Œx¨ _Á?ïDUc£'??¼»g?'3°r­SV?tªP{æ{Û?Œ¶ö¬@Á?x6Lã<'?îu¡'¡–?˜¥Ùyö"†?'ZTº$/?yß
²<H?¤X†«Š›?–A<ñ­?ïþiàÌç'?! Hú#Y?lÀ쩑j?UÃ~0{²?#†Å-î×{?m«Æã?ïȇÝsQö?t:GTJ?\ŽÆa¶z?XtyÈ?t˜_šµÇy?p†(æå?ï­5Ä̼ö?pùp†à5^?rqYÈá?jMCPžëH?vóÃêü'Ï?bE,«æ?÷Ñ«?u¾j>!JÁ?qÒ¢½·?\ª˜tGÌ?€sz'̃?qfL²ÚŒAGN3FGL J0126.1-2227@g)Ÿ¡—ÀT6· ÝÞÀ9'r#3
ïÀ;§èÂ̙?æz–oÔµ`@Ĉ;Î7[@q'Iüο×:A؛Ì¿ä¹-ÔW8T¿ê˜mhÒì¿ä>»×S…ÛAGNfsrq?ïúì†?Cr|	÷?>D_ùt??̛´ù?1º¸>Ü)‹?.Žî°áì?W¿.ª?ˆW©ê\›0?fÿxØIž?höF»Ì¯?‡˜ËåÝo%?"Oï¾N?Ý9Ö?Ž±ZFº²?–XÜþÕ?ˆ! ôÍt?–q«{ßÃv?CU4ýÈ?î=Óø~#? FRàý¥?yÌÄØL]Ø?vùE˜Æ?¨é6¨È0'?žñ8#ùR"?ïü¦Èðãò?5z­Ù2)?.È:1xIÈ?0HH¿ÛÈ?&Ë4	de?!ÀÞ ²m?ïÖ»˜ûm?p)´FՏ²?UÕ,«N^È?TûqBT?o­þ"?i4Û­þéõ?ïR›h{¿i?ƒ"¯^ϱ•?ˆ'6ÄnK»?€M\Nz˜?'ÇïZè?q*ç"3?ßøVF?~¾ZY—êÑ?c¨"'?S[Zi¶—?"&§2Ž)?|4)2s¸AGN3FGL J0127.1-0818@b—ן#FVÀQWü€¿À9§¨Xy=ÙÀ;»ŽÐû«?ç¡J/¤‡@aé;îB¾@²ãàÈñ¿ãŸIÎD

¿áGk#|4¿æ÷Û\S
¿áNL•AGNbll?ïÉXáÃ~ð?wßÞZÛ?goàÞÀ?m¼—Æ;ÖH?o7=/ÀŸÞ?m$àå&˜˜?î½ù¾Ù€K?§Úe~"?†´éÕ^a?'á±éÐi?œæS¢±t? °W
gxˆ?î9ÌÒÅÏ?–]'àЀZ?—<ž Nðw?†"iqó2? Ñ"&ÆÑ?Œ}<(À·—?êo49SÄß?¯›ã?¤"‰œ´?……½#"?ÁLÔ…V?¬t±?Ä	?ïé2æ~œ
?zY 8Nåé?XX±­n±?yUŽ¸¤%¬?UA¡ù?SŠ÷ÎVÝV?ïžZŠ f
?‰ÎÒ`‹?n?cǕu\?z¾wíùÂ?€Ù"÷ýN?"#¾>b¾?ïak®¥ù?{âß±÷v~?'H™Ô¬Z?qÓÿ2…ýE?…\ @²	Ã?o•FÆ~?îƒgc;Ž¡?Ãã
8Ê7?'nôá['®?}'ôR"=?ž$³Ãh)?‰#MAGN3FGL J0127.2+0325@aƒ&€IRÀM ªKÀ9LntQátÀ;hŒ'sZk?Þ8
(Lû@9rƒ«Ë?þce€À?ײÃ%	À¿àPxµÀ¹¿Ó҂4^g¦¿âÔWC~†AGNbcu?ïïƒXîi?Uè\åÿÛ?GÈw÷ Œo?C,ÂulÓè?U%z?NÛ.wÄ?wÜ'?›'Ñf@?~¨"Súø?ˆ3t?¥®ç?—Âj,Ëca?•æ•ÐÖ)"?îçÅ2 }?ŠßžMÂÝ^?p°Ê?€ëðSç•?"O:±l?€C&ºæ°£?éÓ£šh:?«ÖP%©ª*?'f++rŒŸ?‡t¢Àéý{?ɇìñÃ?«› ©à?ïã°žó²?£Ùbì?eÿ-úÆ"?£ÙìLÈDM?ICPE´,?Q+>…«?璉ø'Í?"JþÝ¿Y	?hFÞ¿F/?h´¤çõTþ?€I
TQ™Û?€­BšM®?ï[})K~?sÑ1-šýþ?
Ûҁs.?n™§i"?€£²Ô«vç?c²—v|Ü?íò‡hâ?'»k­Ks?‰gO'WM?o~¬žÓ?°RVˆ'£E?¦{,Û¦AGN3FGL J0127.9+2551@`£ýq?ÀB%'Éä»À9¥Z'"ÃÀ;§YE³Æ?Û
ZÆõó7@­wt«¤@Ìc¿˜ñ¿çÃ&$Ö4¿ë涴BÎm¿ïÿì0€É¿à_ËÌ5'÷AGNfsrq?ïéÏÏ-¹?i!"R¥ë=?S›{‰К?[€Jê›}?XÄåĵ½?`"à·[½"?îpylÓgò?²7õÿb.?‹ péÆ.'?Ÿ¾Ú"?¢LôèYL?ª4ÿ "À?í°SÇþ0ó?›_V"?–ªÍUÃ2?†BTrÏԊ?©¥½›)Ý6?—1³¸F‡?ë$ëqӂ?³…
®ýj?¥°+®éé¼?¥âdAƒ?¼žÂÎFI?±5"…<ʟ?ïöŸ'¼Ì=?UüP¥4Y…?9'‡™¸€¹?CøiV…p¶?Hº¹qÅõ?NþC%
g‡?ïˆ=*Ì(?›Òà¥+O?s5‰Í•?\½Ìýë?"eš­x›3?¦ðIr~?îê8Hyt?ß´oÌ?Œ—WJÊb?…¦¬'õ¯}?"mKC0'€?…î†`Þ?îû(¡£˜?"\ì;¾LJ?ƒlªÍÇg>?xì;)Ý+7?–ä–]ž?ud€U4AGN3FGL J0128.4+6257@_È
€CR?ÙØÀ1D,À8õeQ"qÀ;:-"wú?ì†ëÚ.4F@¯çcÑâ@	/ÿw¿àgÉ<õT¿åÕ=Ÿæ@¿å†ëabpŽ¿ïÿ‰OTHERspp?Øv*\Rš?Çr%ŒV?Ø<è­lÏ?Ȁ@¹"È?Ïà™Ùì.?Á–¶S• ?qlw"¨[?‰ÀÌÇ=?ן|­$»Ì?À¬í€Ã×?ä
hº9ÞY?ÀfZ^è?ß\øQh†?µaܸl}?Òà{Õ'S?²g³É׶?˅²àMÄ?®ÁÓæżû?É('cwý?¦Ÿñèß(Ï?ßsÊ?µŸ¹yþ§?Óø5°)í©?±83iû '?ኃùc?É%Î8æ.%?ÐçAœqT?ğ5BŠœ¯?È	l^ç°Ã?¾°9y?˜ŜìZ?ªã''Ú[ù?ÙºÝÒê¯G?¸g/³þö?â]¨X½ö	?¼«Ã¬l–?çÜJ²ðr?°¿€'}~x?Ū'ùtÿ?¨·xU:êÄ?¼+÷·~~X?¢.±u+ÆÅ?Ù黅|¬#?ªua-¦Þ$?×õ¿'È6\?¯›õ¼Ë›÷?ÌA	Ñv;?£ÁäŽÐáÜMIXED3FGL J0128.5+4430@`;ªÁ	J,À1݆ÀytÀ9ØÊUú˜À;Âٗ¶j‹?Ʀ/UÔ¦@ø|ôGe@¨À^Tt¿ã9\ZÒg¿ç™ë 02¿áۘ=_BA¿ë–ÞûðÉ#AGNfsrq?ïïjö1äÃ?Y…¿ºó?<D4O\?6H/«³d0?Z¤YŽ?Uì™q,ÊX?ï

ˆdú?™u‰î œ'?}«TsŸû?z	ùý×7?–óy×(è¤?–»‰#AÝø?îø@Þ'Ï?‡ðš¹'Ÿ?@AhÉû´?yë'*ç4W?'_—,flD?}ü a£JÖ?î㕰DŜ?åx8w ?r*¸a"?iVèIøíø?ŸÉÍ­·"?"¡c2A€?ïø¹q.$?Aðöx ?2xÛSù?(š@rc?CÝÍ8©ÝÆ?<'º}»?ï¬ø#Æ6c?Ï˜Ô²×?fÂag@?a°'îJ4?~"äóƒ³?~¸mƊD
?ïÐ'JFË?s÷–QÌ?€Ôü*
P?i:ù¸¬œ
?~môÖ~)?e¨þЮ?ïÆâ<)à?gE«¡ªj?\ååŽ@öA?F¥‰,vˆe?uUh¢ދ?dk<ã'ë0AGN3FGL J0130.8+1441@a Ç`|ÀGšÿË&ÚÀ:5O•GûÀ;Â+,Ôta?éÈŒZÒñ@ˆaq´ù@4NŸö*¿àÁÄ¥®GH¿ë¿ì¡ÿC¿ïb…¤ÖIß?êal×n¼AGNfsrq?ïç£ü…2k?oצÛ!ªo?A"«­}ž?CŒ´ !v?cú؆èß¡?míTak&Ø?¹¶£?—ûG¨mï]?i6R¸t?€gè_?‰	Žº''?°Bí)Ry?í0` ?¡ÙQ~B"2? J&}âf?'"£v
äŸ?®sö}œ?œZnl'%?ïÞã¿q^?¢GǦ™É?`ýqã;?}´En(‡?dÞÿÈ?¡ö¼øâ?ïôâè7Œ?[½J*	?'õë;ÍÈ?*9>`äcá?S=>·Q‹?Y<e壺…?ïԙ pA?~áâɑl?W¡\ú¤?hş™ÔK?oæÂ??rÓ§Òi?îÆ`¼OÉc?Œ
…V?ÓŽÒ¶K?€i´Að8?˜J!mUFm?†(0Sb†;?ïáž5_³D?v†6ã.t›?C+G'´xÖ?_ŤJbë?i–ø½\¢?sÑӞLÛAGN3FGL J0131.2+6120@_ëğס<¿òµQ€¦-§À8w3¼ÅîŒÀ;§' Ö9¿ëëQÑ?3ƒ@êÍ–*y?ýÊ€¥+ô¿àÈSõlö¿â~zm?¯ª¿Ùq¾óŠ°¿Ìsì.›AGNbll?ï´/xyʃ?'ÿÖfŠí¿?4Ç"5-Ð?6Açèê'h?'MèÛì
|?'¬åLZ¬‹?ÕIÿ6›6l?ÕÍîž6iý?¥;¥;œ	ø?¥Ád}œÒ£?äFKÊ?ÔýænÎ-º?ì"ëíFj?¤·˜9ö…~?"Ÿ-m¦•Ž?†ˆÍ†•ŒÃ?¶0ÛÃtYO?¢Sºʗ??ïæúlå~?Œ@oÚùù:?q€‡P~?">©žæÎ-?Æ¯5éð?Œ-󆴊m?ïêùõ÷i?c@mÎýŽ?-üǃIÎ?,á8§ÙÓ¼?c&¥€_N?b%Çìéyã?ߙ÷Ê?Ø7Jc?YK?¨ÎNÀÍþ
?§ÌTT—v?ÝL?[Ö?ÖE‰øøàã?î³ËÅ¡ñh?•à']í?"w®½_´?z1EÑ%6?ŸJ°Hâ?"Aú] 9?ï¿Å0 Ý?g»çΎ?>v.à">ý¢âÞ4Š?ðÿl"KO?g°&Ê°˜MIXED3FGL J0131.3+5548@`οìºÀƒ<ŸÃFÀ:=0l¯VÀ;šºZ•¿ñ7`Ú5k@kÏæ1Í­?þv3þµ'?¿ëΐŸ‡¿Ý€Òõþç¿á#qKòœÀ?¢ÔoÁAGNbcu?ïÒvpA(?mlçwú·?A衬3zÉ?;–Œ¾S&?tµ°Ÿô=[?lQk¾¦)±?îwè¬Í?®c>¶4Ñ?€B$¤Ö?‡Ñëj}¿w?¤pô¹Ì)?ªñ¦&•	?îÙòz0s?Ž†rë?.Þ×ê¡Å?z6@Pù|ä?Õâׁæ?‡°MœE?Ànçâ?}ÓȝÊÍ
?3¾Z5`Ö?!7†Äÿz†?ˆk¨\ºr?}¿Ö五?ïî#RÚ1S?URËnÈÉ?2uµZB7å?)Øó,Tõí?_ìŒß
¸?SÐn"ː?ïl2°MÝ{?Y±J…ø7?j±A£äå?r°ß¦‰¥?ŽG…׬
?™vž—~?ïh;°&Æ5?x{‡¬Òq?\@'o*?kسòH¤å?†BóßO<?pp7_òh?ïíTŠ×ðþ?SÕý¯la>ø%Pq£¨>ø"@v
o?bzW¶¨g?SÁS3(¤AGN3FGL J0132.5-0802@bûw µíÀQ%4ß۝JÀ:ˆÉûaÀ;¸A›«Â'?à :M·³@óˆzãK?üÚß_ ¢¿¶S"F@g?ïšÎãõ«¿ÚÎOT¦ö¿Ðà-ëSSBAGNbcu?ïëš2EÍj?\ËCoG^Ú?Bùæµ¹–é?H)O"E´H?_N§öY.4?Wà+ŽKJ?ï=O;|'Ý?™œ­ÜWë`?uŽ}õ	ë?~p.·[ ?"ôøUŠÎ?•0:M·³?î…Ý®¿ú?Ï#ßÆ32?'>a(F|?ƒ¤
 Þ÷?žû]'$<?ˆ®Çf!P?ìÀ‡a*3Ó?­ÐÀm '?¦F$œTzz?¥Ÿ¡8§ïÑ?­±eM˜¬b?¥üÃÅɵ?ïõYm{ûÆ?LÁ˜qN$?1Òmu'?5!ÅÖ'ÁÛ?PØ£ªÊ…~?Ghò|ȟ4?ïÂ+ÎåÖ´?€ }Nan?`ô«í8?cž"¢‹e?vàxt?y/ûôï1ý?ïIÒ*:;?€ÐB¨'?"k¨P[Ú?{xéµ	?‰Ô43ß?sÔ_²|óP?îÿk!®rç?Œ‹‹|V?ŽgÙñ¥?2Ɍ–Ü?Þ®Ñ®Ï?ƒÅ"½¤pAGN3FGL J0132.6-1655@ed@ò8—ÀSÁýaÀ8]à_PÈoÀ;Œ­Ánʹ?ïj
®ÀÙ`@홟£ÉÉ@pê¿üÚ²¿âðƒÑk¥¿æH @ÎbŠ¿éQØXNÔ¿â—!B¬BAGNfsrq?ïû¸¬Œï?9Ó^$ŸÂp?/¾ki2|U?,)·"(·?7sØTÆÓ?0Ô8u(C?ïÜ §ÀN?‰Â	" ÿŽ?eñ(™u¶&?sæXßÌ -?†L­±Vü?ƒRËrZj?îö…
ìK?‰Û`»?ŠQi£3€ž?{ÖàhâIè?"¨.À"U?"i¢¶á?ïKúäڂ?"úºËâNç?[4È)g
?`¢ß®É?"ÍVê°S?"£©ò…?ïýl…]?*ÈOðêm?#OUUý›?f§36"Ù?&3µÎ
ý€?Ò\?ðp?ïÜ4‹oVÇ?kˆÂƒ¶?Q'	ž|ê?QO-Zí?k
oãÇI?e—ÏýÊ??ït™HL0@?yP—m–ò?~ŸXŸý)˜?iÑw1ôÍ?ƒŠ¢Ì±?snºTøô?ïà5%aõz?p'³&"?E€Ì4s¿ˆ?AЩ>ú±?jj§m1¦ª?nòÆ#—âAGN3FGL J0133.0-4413@qy[À6ãÀQ½²_Μ±À:/ĦãÀ;üË+­-¿äP/5€H@@$³=°@?ü¿ÙŸC¿Þ jpX¤ÿ¿â~U<ê¹i¿àÈÇL/Xˆ¿äJ‡áò_AGNbll?ïî°©Dv@?fñ{—ÍÔñ?8b"çf~?>u/(Jð"?\•M>Ø?eµÁ¶úâ?ïyndr×t?áœ&aŸŸ?jìÕëTXd?pL¨I¿¢|?Šé1mœvÕ?ˆD xBøF?íÛ
'«é?ŸjìTsí?ªó«€CT?ó
l5N?ªä™ênÀŸ?ž"
U"=,?îՑBq??'þ´¢õ½ü?ZFæ` ?Y…7æäå?¡Òt0ÈWš?'…ÿ"0c?ïøñ™hyð?Sˆ
ÞÿÌù?%å:íV;"?)0_Žx¸‡?FÀJÄ?Qú³ Û?ïØòd?qh–‡s?T*ÖXiá	?T%)çÑQ>?m梚IñÔ?kvô>-õ ?ï3t)P9?‰ }8é?ƒº)Sì?ðâ#ø·õ?•¼|²(ß?,´j¶?ïÆÄõèÏã?o:R&Šxª?<áµ
"Û?0¹Ò'äMX?zÏi»¬¨8?ngc­ùžÏAGN3FGL J0133.2-5159@rˆv\ÀOö¸¿ÏŽHÀ:pƒÇ ="À;î£~éпÔâHæ_R@õö`X@kŸ`X¿êu«Èg¯´¿ã8c‡'Ç¿íÁ5
—±ý?ØJÛ~SÌAGNbcu?ïìo»{ß?gÂB8%`?S•öAPZs?XdµþnK?SŠ":†˜ô?`(¢ír?ï©!å"Å?…PyÙσz?`Utr¸ð$?g9ÿI9@?¢)²—F¢?¸Îk¨?í²¸uÁ'õ?œDÄ¿²éê?›Å"NÆÇ?£Dý°Ña?¦ñ¶z˯3?–ᆔÅy?歷YCY?†ú¤8"v=?3#±Œ%?C—¶pI?…ÃÑfꎷ?†º7?ïô,zå×é?aÜfk™??¯4÷m@Ñ?EcaÚÕ?OvyJ¼+€?["aÈ?ïâWxi8?k'
áÄ?L©aQ˜gÚ?OðNï,.´?f~/œ'¤?eA¡"ÐVì?îõnSg'¤?^IÂ%[?ŽÆpØ©P¦?"Ð#ÿ'?'îý*5ÿ.?ƒ7Öp»…!?ïõùDc?VâÔ¾Ž;²?ˆ_Gi¡{?ÜØbÓH?Si×~_Œ?VžÂÈÆé˜AGN3FGL J0133.3+4324@`^œŸr÷nÀ2Ш߇ºtÀ:BЏ±¹À;Ԓr]ën?ÞÁ4]·ñ@¯ùO·£@h~€
¬f¿Í´›â&Ú¿éM$ÓknÛ¿áËÈ­zÄd¿æ9'%y-¶AGNbcu?ïìÁ}t† ?Z<î#-ßf?F;"	Óç¥?E*»;?[_B‰&)Á?U{Õ<ø£Ô?î™hNüp?©u(õ7g/?†5ð"*³–?ˆ€‰.:Ɠ? Ûþî´?¦gô¡Ÿ?îþÎ/V
?nÄc.¾þ?'n»1Š_Â?'­EÂj;?Qk
B¬«?"ó½æû®)?í–âú²?Ÿ{¥}²Æ?Œ>ý/¯ßÆ?'²ºqêIÔ?¯2"€Cë?›À¾Ïó˜ ?ïùžeõìð?B֊¯ù?.AGƒO‹?1"di½º?B—û@Óº?<ŒÑrÃ}Ù?ï'Ѳrk?´ÿ–?mïÒsa?gr&ȨN?"žÐ-‰	?‰·&ª:†?ïkžOs?y‡®'µ?-'úqªû?s·Û f?ƒëDJ1?l`WÛSÔ?ïfªWñU?yüé4‹q¿?~
W´?bÁð›v"?‡PhÛÞ#?uaäÉ[9ËAGN3FGL J0134.3-3842@p¾àP7PÀR×"Àh¡À:E©¸ËŽÀ<jüY'¿è"íŒò@tM¿%šC@¦H «L¿æâ.ÝdÖ¿æÚešA=¿Ð·½å4¿ëøÎEGݺAGNfsrq?ïì‡d…2&?]'õÉAé4?RD©Ÿ˜ƒ'?P´š|D«u?T¬Ùô/ï?Sb*çÄ?fK/÷?ŠÚ¢#?eF¤`'J?f<Tnh$Ä?‰Àý`¾[Æ?‡–Öq®r?îuðA(?'çRrÈÝ?—,Âge?†
ªË<¡=?š/ÿå…?…"÷e«;?ïY³W°Àþ?ŠFB¾óC¥?HÿéˆbÍý?XÃ[ù<Ϻ?"•»ÅfÈ?‰O÷AÉÃ?ïô~KNK×?SU¨ê¡Ÿ?E¿mPBU†?Cx~¿ëF?HGd·+Ò?HM¶û\¾?ïØG6‰)?o°"/A?S{2&t8?SÁ '¿Ý<?mûU'Æ#?i¯~G­?ï@uà	ž?"™•7ö?‹V¡À|Â?~>ù¼¤H?"¢Ar‹ïª?tˍyŸô?ïãZ~Œß?`©}ªø?/I…J—ø?'¸íÝ™?j°ïžv^¿?`v|ïvéAGN3FGL J0134.5+2638@`׃¡	ÐcÀAŸT_Ó¥.À9bÒX'ƒÀ;{"qê('?ñÄmO¹¦ª@>¿Ä¦Ž?ÿÛg_4Ã×?ÑEÉïˆõ™¿Ù؀	O´ô¿ÝTžg½1¿æí¤èFÏAGNbcu?íûdAjzê?¦»O•3? ü@…e¶ç?šé.3BmP?žšöÐ|:Ö?›WÌ<%—Œ?ëÛᙧJK?¸'NM×(?¨SšÍv@?®6t"(?´÷kæ¨Í?°0q ØÝ?ëtµå]E?ª*·yì‡?´Ç'å©æ¹?¢ܞòŒ	?¯%›ák—?;'jdç?åá—Œ¢?±}Š
Û@ö?¾rÍ+[<V?¨¥k¡&?É?!÷L?¯ÞC¢|l?ïb,{Å."?ÂFÁBpŒ?†²ºãýQ5?"‰gÕù²Ž?€Â&1î;¿?Øö´ÑP?î¾#!ÿ??±^(Ì1YZ?š¾F9YÅ?¡D´Å,
?¡r>¨/ª*?¨(k«‹
Ú?î(D^Ì
§?˜àrF=d?¢P:髗Ø?'"w¸÷—w?–VþQo­d?†¶žÝÝ2¤?ëZZÆí\1?žZžºžU?´ã2	£©?"GQÌq?°J""e¹T?•ù‰ÃFAGN3FGL J0135.0+6927@_°ÄŸ×¡<@¬Æÿ®K'À9ºGº©´šÀ;O‹Ëz½?½I¢z,°§@Ó.ö¸ƒ•@tcßÎ\D¿ÊIÅëKô¿ëÂsÊý꧿å¾ësè¿äU÷i"ªAGNbcu?ìjž´fz?½ŽX!C
†?I³é,s?'Ë^E'+™?¸˜¢&²¦™?»Þû¬ó ?éÂ3=
?Ê=–£ðà}?¢â•{›ºƒ?§¿,Žôè?Ä>­/×?ÆƲpCú?êlh£Nñw?®š'>1‰¨?© .ûic?"ฟÀ»w?¿Ì£iA?©‹ÁTØü?çѼˢÖ?­Ô•v+? ôÕ^|ô?"vÂ$‰??ÏG™yÕj?«ã¼Æ'Â?ï%;:‹
²?£0«ËH´?tF
ÐØ?€æt¥Û§Ÿ?–X˜oz?¡1mV=Ñ?îfHû¶3?µLÿ‹[«\?ˆ-na£²?'²46À?£Â|3O?±mŠHÎ
?î(ÕÁ_}¶?•Ÿ#1¸}Ã?—ˆןÄ?‡3Ó\­ß?¡è_äð´?¾çZ7q?íی¿QË?•Á3u?'IÍÓÕz?xu¬]Î2Å?³&°TšVÆ?"¦g~›bAGN3FGL J0136.5+3905@`9à`þHÀ6ñ§Ši{À7p͔ré,À:sˆ¬Œ%?çKÀÌþÓ@‡&°:?û!/à˜[¬¿á:p'2¿×ᾨ·¿ÒËjµ^#Õ¿Êþô^®ƒƒAGNbll?îÿžú½²?¢D6ðêÔÄ?pÂâÖÁœ?w©SH˜õV?›Ûš±KÛÙ? Ãõ©ýÏ?îÅÂ՝?¯D7EBO?"Iå6†?¼ÏDD@?"ʃ'e?«	‰äÂMG?â—™~¬?¹Låìô?±In=Ë<ª? wS.âQÕ?׎u=·?¸h¹Á.u?â"íW±Â°?½;—Lô?…¿mo˜^ô?†üÿyÛ(Ô?ÚH)åV±h?½všn´FL?ïVP¤6? 4<Á©'?k´Çí-?vñKp7"?'¿x}¡œ?œw$UžÞ?ïv×åQz?œb@݂áù?u|
iåiÙ?'ž•?ädÎ?‡‹ÿó­Æ©?–‰dbîX?æŒjÿIÄ?´äY°pVÇ?¯Ê=…¯r? *
P½¶?Î!tøX?²EàÛÅ?çèáG]?²bŽ¤Ú?Š«1«Ø?| >êA—?αȚ8%
?²1āÑ[:AGN3FGL J0137.0+4752@`Yi ­ŠÀ,˜¥ÀïHùÀ7²MryšÀ;ªÆè‡=?ú"ç÷²@WK@î>¿àä-R.Ý¿ä¢jT¡[Ê¿ãùÁˆ(¶‹¿èãÅYÇ¿AGNfsrq?ïí¹Ÿ¶¿?U¨‹@7Ã?L»ö2foÇ?GÂ`YÞ'Ñ?V/óuž‹È?NÆA ~<™?ï|¼ä¢V'?æŽCË?p•‡
¥:?€R\ðÑ à?ˆ†C–ü²ù?ˆ VzŸ©4?îUP]Õ7?›.
ēâ?œ½"Âì®|?" 04ÕV?˜Ÿâ*yrª?'Í$Ä,*°?ïǍ^^p?€åÌntO"?@w¨¯ž1ñ?S(³ØÕZ?z*[½zÓ;?€Ä¦4&?ïõxYéÚ?KBʹ׳Ð?GI¬Û|î¥?Aޜ÷ ïÊ?BÔï¹q:/?=˜ž¾&D:?ïÍkm-Í:?uܝ[7?Zr¦¿µ?Y˜f×»m?rƬÂÙ=z?q»gƒ("?îÿ€'Ïõ?'ÎŽH"v?"+qÛ«)?Œ'¬Pð?‰ÉMÍwÉ?"(e²õ?ïôwˆo:?[ãˆJ¸?2{=O
—!?2¬2† 4N?Rr  4gŒ?ZDjPË[sAGN3FGL J0137.6-2430@i,ÀÒÇÀSÑÒtwÀ8柱mÀ;ÀØi¹>?ﯟ%°ÏÒ@ŠVf/]@$ Tä¿ã@ÎØk~¿çCAj¦¿éi¶¼Xû¿ç¾ãèÈ*ýAGNfsrq?ïùlÉEÈ?BëÊ«.6?7"®f¼?=b<pS¼??ïêüoÿØ?5K³º†"ø?ïwïF/ h?º‹sêr?mÊë`2³?Âþyæs"?Š's'doU?‡Úwøb'k?îï©)ðŒ?…ÓjÈ6?K?Š,èI¹e?v kš µ?"ôiIÌ?uoaÅim?îí:¸ã‹Ö?œ‹ýI?u*jWyÈö?t]LˆÛ?Hˆ©?šáàŒ ­?ïü¦l™cò?,97m¾±‡?(Mò©%"G? Œe:"z?-KE¼•)u?! âs€`?ïÐãÜ×\?r{7áõ$C?YÉ
d£¾Å?Xm(z¸¬?qõY~æ?lGðHFP?ïw&Ëyn4?u¶þ5Mà?k÷¯»?j~6^Ý@?'€Q¤Ûgª?k­áÅÈÆ?ïËåò/)?yš"Ÿ?Z?`lãŽh
?Sð8
€0?r=Ì.ŽS*?wŽÎ'‡EAGN3FGL J0137.8+5813@` Ç1¾À\l.NÀ9Ý:ZMÀ;OZˆ%¿çê3!añÚ@Ü¡jHs6@u8_—ë¿Ú¶½Œ'¿äå?æ'šV¿ÞÁ¤G¿ÜO³7‹˜¶AGNbcu?îێ±‰$?¦Ã3Ïmïz?pyOÞ¢Õ³?lÂ,p…? 7êëÛU³?¦juBâŠ?ë""&è÷ü?ÅÀ¾¬M¦Q?–6©ïc?šÓõ:H3?Àµhe?ÃÕ,µÉ-¹?ìô§Ÿõ0ø? µµ"X{?Ÿ£Y¯ö\¦?‹ê6êø±Ø?°qì"Æԙ?š=œ¦eñ&?ìòyÚ
ž?¢Ùvö£Ø.?^‡™Ô2_ä?[ÿêžfr?·òÈØÂ?¢¼×""§¸?ï™`øyŠ?Ž7لAøÜ?`ûvZޞ‹?Zyjîï!?…häQà?zSñ(R®?î~éÊ*þS?±œ,Ú1Aõ?€"µ·ºõg?‡*¦vë§?£ì5í©|?®‰¡¨&'J?îé­yå?}¸]A3?Ž"£žFd?€a…ú?"ÌXŠe0?ƒÍ& ½ú?ï-EÏd?'EK³b'?E©!ºµ¹?9#ÁïÃ?™¡†K"d?Ú¨ìFßAGN3FGL J0139.9+8735@^ß/@_k @8ÇÞàˇRÀ:[o¨.‡ÓÀ;Óác\ƪ?ÎcJ]'@
èO-°7?þBŽ_Ô¦á¿î¿?97z?Ûd˜nSù/¿ã"=êZۿŬ†6́	AGNbcu?ïóãíOÏ ?Kk¯~ªª?9ü(6­I¥?6\+ç‹?¬?Q¹qã?E¸Ô*?ïvà–%i?—ë7(Ý°$?z"ʲ7Ã?ƒãÊGÏ?"þXŒ¾QÐ?"¬Æøˆ¥?ïLñÚ	?'ô¬¨?†À̌þ.?u×öÆû7}?'¶t4ŸÜ?x
Âþ?ï9èÑ\¡?"?4xv—?Šè0,L÷ñ?‹mùä¥4?'DªÑe½é?‹ÏùìMm?ïú{ƒ{l?6T‹Òõw?(cóÐp?[2e°n??òWyÈhé?2²zŧÂ7?ï×·§Õ$=?tQ5ŋ?b3Q¢õ7?`ð{gÔú?f.$ÝXUð?nŒ¦©õ>?Š™Þ?rë
ªŽ?y—9E…–?l<Iâk'h?€'!¼N‹?bt%náùq?ïÌÄH'5¿?l
è
|5?g³Ti°f?[Ā"?‹?kˆbþ:¢¥?d£jΌâAGN3FGL J0141.4-0929@c╁$ÝÀQ19Ü>ZÀ8~ê–pÀ;Rùþ?ÜágfÊ@\ÀÃÕ@ûª ¨»¿ØòvÅf/¿ä1Q÷zÜ¿áh'N4§Ž¿ãÑi—H[ŽAGNbll?ïúUkÂEà?@Þ"Ù?íø6èwÑ?M^fj}¯?D'â¡ã?>a|""Îï?ïp~"¿÷?Ž55ÁØÒê?nËo
®M?vp^Ï{£C?ŒHĖ§´«?ˆ6¸²N?îÙkDF?'W¹•Üwo?†Ñ¢8hk?{<vˇ×?™sá~S¥Á?Ž^~z)Gê?ì Áќs?¤Èzײe
?x?î/X•;?r7ò‰™¢ ?¹uò'D•Ð?¤wÔ¦I¦?ïýÎï*´x?'܋w¼?
"""y@?(HG\x.?+°2Ãè¹?#ÇÜ:Él?ïÈùÐLD?v"û}?]+•`ù	Ú?YMòäÿí?t²Û{2?q¦èÚµÉ?ï}Ïõ²Z?yÕðæž6b?v©–ÆdU¦?lè¾6†JÅ?€‹Àœ¡Ž–?sTÓ!hÆ?ïÛ/f?‡pâ[Î^¨?h'üæªÍS?Vl½…k–?›:t'ú??†Ùú_t]AGN3FGL J0143.7-5845@r'@$³>ÀLŠ+¿¡kÀ9)–‡å<À;h¦©L•¿úÊ+lë:Ì@ƒ§>ó±?ýj*þÜ>…¿Ù²ðm:ëä¿Ú`%¸)¿âðZ›ü¿¥Fÿæ!)AGNbll?ïùFŽ•ë ?<ž+Ü '?"¨Ú¢%˞?½ÈÛ§?F;1Ï()?9fD€Ùt?ïªÅ<ô‰?ƒ?~ïîì?`"eK"pç?dï$j_p±?Frń?ÒO"ñ%?ïã¿O>?‡®¼R??‰`áðŠ?€o°âˆ´?ó"á±?}2~´9MÂ?ïŸúε&µ?}Áµ{ÿ(4>ø…€²•Ýƒ?¢.;žÇ?‡õ	[DZ?}º´º8øÓ?ïû—!ç}Ê?4éDß¸H? :'TäN?@×¹?;)ÞlEêc?2£ÛÖAÍû?ïâЅÐN?ht•Ñ?M£p©†?P 'cŝ?eƞfSj?bJkáµõ?ï‹lvº‹F?€£ÜÉ..ª?}˜ô`Ãô?|ŽØ~?|°ÐS%R0?q'ÌÉWY|?ïìfÓ§:?VL3SÕ4>Íô!|+DÆ>ÎIžo»Á?cê_Mj±?VJ(Š¾*AGN3FGL J0144.6+2705@a)  ôØÀA%ë`5ʽÀ7ÙcaÏ'ñÀ;a$WÎ?ò†¨ÀþãJ@D8"*@kïð=jD¿àK\øÜþ§¿ã_Š±
Bx¿âÕAVÛ¿ä —YAîAGNbll?ïì›5óNc?fC:?"/äWB_? =wÔ™?bA˪Íni?eçžÊÜãÀ?ï+Œ#Ä?˜‡K·±A?ux{|!2†?{T=2Õ.4?•0Mn«€ã?•ØãeÓ_?î­êh¶o5?–¯>Vê6?‰¦ß
8©o?€_§8ËCý?oCjôü¨?'…©Æº}?ì×B®?1Þ?¦×Â	ªl³?"V¢'~T¿?a-¨íè?¶»9¼ßü?¦Uð·Q?ïû0֎?@2ÎÄ?¼á%…Nƒ?™Mø…´?@'á¨Þ	?=œ°/ºžŒ?壘£)×?"l6<°"?gMÌÈåFt?f.0Ö;ÕQ?€Éä<Æ«?šqSQþ$?ïPø)‹®c?ˆX¾Ǐë?€Ë7—`K?wBºm¯Dù?Šö¾3§Ý?ƒ¦;õÃÌ?î÷óì÷9³?‹-5iڔU?}1‹ÂY??j\™IÙo?™µp®tå?ŠÎÝÖÜÜAGN3FGL J0145.1-2732@k>àŸèh4ÀS"2_Μ±À8ŒpUÓq,À;«ô5Çb*?ñâçæٓZ@ýˆšBáÒ@Ž'`:'n¿äs'¹áÁ.¿çódÑfs¿èîÉëਿì(LQ"™AGNfsrq?ïì˜>X^?YÀyICs?UKp³õ¥?Q¹µ-÷Ǒ?R{"šp?Hæ4aP×<?ï"h…ƒÐ?Œ]ø©€Š?iÙç_C¶$?tVW˜tØÓ?ˆodÅZ[?…ÿmršp?7®1?'a#ê—‡?™nìëØ?‰0£è¦<Ø?'£ú!¸?¸ïÈð2?ïZ}ÀRɄ?"ZãëI?h<CÄý'å?lAŠ÷XÔ:?'¨¿x碅?"L{Èg&D?ïñwºTWÏ?STï2·¿?R¦©Î?HÝ8U¿Ös?DÓù{ðÎ?E#3ÂXÓ?ïÕ5C%;?p²óc¹?V\
¡#M?VSÊGd(?oœ¶'‹Ý?i"?ÆÀ?ï!Ím¼Ø?ƒ±pMŒz?'Žï¾áŸ?´@T¾6?"nÅO"ݶ?o¨y©Ã?ïÝm'u?vCkÃ},Î?Rž
ƒšád?Un×!-,ú?iCÓ׿'T?tãSÞ¹³AGN3FGL J0145.6+8600@^üá~4¹E@7<ö í¦À:@yꧩ'À;Ú|öË£Ø?ÍÏ·úKO@e™
©@&«?ß>¿åL{7-ê¿á¨å¨P¿æØþ"¿æ¦_&oðAGNbcu?ïÛÆ1I›w?jåؽ«¦?]ê¢Q¢TÁ?\«þ2	çY?eD}}>Õ?c>Ö\r«?í¢Ì"l?´ýCéÕ?¥%VÀoàý?¥x"ÄG£? ­à?Šw?­gì>ÖJ<?í¯îÂb]?™b£IåY?››* Tî?ˆ8óXÖ¢?§3~‹åëœ?'Ý
c"n?êbzØu?ª–áŽÐ"?¹×IŸÓ'Ú?¦@˜—
d?µU¥äUª?¡ -¾qmÀ?ïôíÚýz?MÓöA3çI?>qb}¡?9X`‡0ã±?M<8öÒä?G¢D%ȶ?ïtHQÏ«?–dlÿQú?'µŠ ¬%?"Vۗ2'™?€8ÙÛ<?+>È{$?ï)óàÑ«H?€©cîìL9?‡4†}…?tˆ&B?ŽNû7Y¸¢?tO@X­d«?î†ÀÈvj¯?Š.œ¸—gŽ?œßRÝ£-?€ûð•ð'Þ?'H"ڝ8î?€Hîi&JAGN3FGL J0146.4-6746@rqú?̞ªÀHB=ÀTïFÀ:4Ò{bvîÀ;÷õy"@"¿èzjÉfT¸@
ÂPŸªª¹@ )`vP¿ãµ¡Øà׿åFGž¿é=uó»è¾¿Öb¤æåãÛAGNbcu?ïXÞñg‹Õ?"úߜŸÌ?câ6Nš9¡?a½ù$‹Á?'gÛçÙ'?" "C–ä¦?ïu¬§¾J~?'#zç#{Š?k2ÀËMx?zyþK-{'?‹ÏIm¡?Š¥ôÈs´ž?í1J4)Â?Ÿƒª2Ðá?›ïkÄZs¥?†¿ƒÔ"}Þ?®ó¡-ÿÆ?™›Ã‹¸¤?ï"[wÓ~Ë?E]åK?R"Ã띐?Uz¼=lIæ?šŒDÊÉã?ëå4,?ïؒ#|\?sÍn`v'?G-bÕvÓ®?Eá‰L6eË?pÑEaDq?ršUE«?ïס7+?pŸqÐï?T¢50 ̯?SÞÉù#U?nšD~^ê?iGLÏJXN?ïÔ ²?Î€gÖ¥?‡Ä6ú]Á·?qñ@ÿ_€H?'Â(Mï?xï´ñÈß?ïÜ9µ6
Ý?iunS´ã?+ÉÙEÇ=0?"½'"Òõ?qÖ°N²ƒ?iß,ĄAGN3FGL J0147.0-5204@q¿?á—_ÀOz-K6À:=ƒJ¢»À;þ0íÖ¿íÊ֗?»ñ@:9/K@˜¼ R;¿Ä¢¾lô¿âð³¡á¿ç†kEÿÀ8
{Œ›ãAGNbcu?ïñ ¾4À?T—ºyÄU?AÃzãt?DEûñ
?SÝ#€él'?M™‡?ˆ-q¹?†-£ª©1H?ajæËu³?fEÍØþë?ƒ7$7wzˆ?'͝ì]`?îŠü9eÁ?Wœ¬Æ'?•>¦=rÐx?"W$'ò`?™aҜ´E?ƒ'¤†]`?ï'
âýÌÛ?".àñýrÚ?+tˁùE?5›<H¶?‹Pmy×¼¨?"ñœïsC?ïù…iœž?B"¤¸å?/¤¢{I?.¹ÂÙ^«d?Bžæ¹Ãã?<ÄðîՕ?ïá.¼ â?gõ¨ã_r™?N̬Q]ä?PQ"!)£?gü¦M?aæð.7¶$?ïRý­F¨?€|#Jq?†Çh¸9è?xfîrÎ!‹?"yUÊ>{?r"*»?ïï¾eš¨Q?X`™´y?ÀÂ.‹À–?‰ê¯«M?_í.[Mÿ ?WÍiŽ'¹3AGN3FGL J0148.3+5200@`xwß (À#Ä9 1xÀ9¸þ›{ñéÀ;%îÇÉ?փՁò"@cFçp?üRóÀ+©§?ïýìH#k{¿¿Î'¢À¿ã¢+e"]g?¥©yámmÂAGNbcu?ïÈýtàQº?xë-þp?c\Ž.€Ù?q#ZÙã\?qÒþ|µ¡?m°Mk¿Õç?ívR¨LŽ?¼Ö'®3žW?‰Ñ\9Î?Ñèß_Èÿ?±Š%+ŠR?º4–Š›yï?î<¾‰	Ú?"'bÒª?"À¨v#?"
'X¯?¡ÓÃ`7YP?ŸH=*W?(¦½?Ÿv~~¹ƒ?hn(ìuõ?rŒhA©‹ß?£À<NB‹É?žFÈÊ]'?ï܇''Ç?›[»z…{V?d¹K2|د?›d9`Tñ¢?]~DÛO''?UXQ A?ïJ™?œISœdn!?pÊ¢à!»?s¯ç"D_?'‹VȪ!~?˜´
'Šä?ïÈÓõF?Ž0×CþÝ?ˆÝÿbå?ÜÀšðGÚ?¢îgT¸?ˆ–ÂU£Á(?ï¾ûÚÆ#?{œWâ.¦¹?L#Ý̾C?IF2?|ý–éòêœ?{»ßé,AGN3FGL J0148.6+0128@bÝ"ß°Õ ÀM †¿¢AßÀ9ÀX·Q:…À;ŸŽ'å".¿ÙXim×ÉÖ@†öA»6L@*@\fˆ¿Ú³ßæ…·¿æ—Oß³§¿Üvpd_¯¿Â•Òÿ[AGNbll?ïôÍA"?QÇì"0Œ$?,)q2†0Ï?+J‹M?S?74µ'?O\⨲?ï¤óª\4‰?"—݅È%?`¶¼—+õa?eô¿·'âF?'•fIW,M?ùô§?ï<ÌH1`å?¤»Û˜'?}[2Vm¶?m	°Êb
?'ª]…C?|âÈXÀ?ïi?l&™È?†3q¥z"?ÚÚXx×?$Ëþ"çá?'»8b¸€?†(ÓÐûoG?ïúD¡'?D
¤d°‹º? ÜoIœ-‰?Þ».s?B¶`Ø]Ëð?Bd'¬'©?ïâ·¶¡M~?hEVá5'?L¹Æ»w;™?O²l±©Â?fן4?bx	Œ}ʯ?ï¬fƒþ¸é?m"m᥏?oc¨ñÑ>!?b6f˜_7Á?zé€+ÈR?e·°£â£?ïåIêÉ{Î?\›		)ы?ˆ0ƈn[?·c ± 
?j;ôpRj?\wyÝQAGN3FGL J0150.5-5447@qÚ®_ú;›ÀN(}?Æ¿mÀ:ÎakTâ°À<*'ë"z¿þøYÐÖÇ¢@CpcÀCÒ@ò -1'¿íïÔ.ž"¿Ý¥Zõfkf?aBàÖl«¿è2£Ý¯AGNbcu?ï£;ÙÊâ?˜eŠ]Ø?ƒºãä<?˜v<3?`…:c"?_Ô}PNÖ4?ï–~[z¥?‰~é|÷Ež?d·´y½)?r¨ZµL?…Ks@Ëiy?ƒ"X€?íìcÇÇø? DÀk˜ê?¤‰0?D?ŸEiÏNÉ?™k×+¯ã?'aÖî?ïËÓ¥ÙîÉ?uvnpïñ?"RB–A:?;Ï*Æ­?yå~ `­?ub©Q¢Pú?ïÈ=BÍýF?ŠWHª°ò?wå#«4Ýf?Š)L^æ/î?Oá×%Ò¤ ?Lðh•©…?ïޜMS?l6qŽ0,Š?P½'u]LÔ?Q~Söa?iöVÞ/?eÈ0›']?îÔ
ãcá?—/¿ÖÝ+q?›(ìO¢iG?–»p©ÂMñ?"ª®'cÅ@?qï]*‡ë?ï÷wí禎?JXÚxÞd>ìÊ5«r¿>òûsÆAjš?P×äîx	?IÛð³µÜAGN3FGL J0151.0-3609@oƒÿŸ‡ð$ÀR†À
¡©À:mtòd/À<gpQ¡³Àæl¿@+-']¶@¬]·ñ¿çųT
{¿å5m:ž•
¿åžçsŽr¿Ö"½.t1«AGNbcu?ïæRóþü?eL8™úÀ?;ëŲJ%á??ϲÍRy–?f/"Už?c™%õïÆ ?ï©êJ>Æ?‡>ÆÒFe=?aL´c÷W¯?qà,&ÙÆv?2@PÉb\?Eï&£È?íêŸÛÜ?™*$¢¾ß¹?—îïDBx?'æ4ÇÆÊH?«)ær),
?"J$ÁtaÎ?ïºN,1?;b6=@>øuû¾.¦?á…q8ÝÉ?`?æö
?/³8Šö?ïôw‡å«Û?QôÀön ‹?.¢‡‡ÓÞa?*®2'­?S<Ÿ´/?Pv†º?ïà‹Öjâ?o^oÒwV?NB$þí?S²¸xÚð?gîfo1¦j?h|\ô'o?ïc:~\?€F$/<â?…(o:"ê?m˜Q´ÂXÄ?'¿a"†r?wŠ¼uGª?ïö.\¬Ð?KŽÝœ&>³ñ¦p2>Å9ÈÆ.æO?Sžg.É?Jÿ‡ŸÈ
AGN3FGL J0151.0+0537@bœ] l‡ÀKK¹ëÀ:o¢äßÀ;Ӓºǿޔ®tl}@
w¼'&á@@ߜÿªšž¿ë<TÞÕ¿âA¾¦:ß¿ßlsñTl¿à÷ŒŽ™5qAGNbcu?ï¯ñ™N´Þ?˜µHHY3?MsÚàA½?MLI¢Ç°­?',[ïe69?˜†û(ÖT?ï{ò±&ÂÑ?‰·`?hþ¶n‹?qbò…‰8?Šßþ
]?Š c˵?틇ÎsŸ?ç2çyo"?—8K^Ž†?'gq`ºßË?«±ÿÝi~Ô?˜¯¿ª™T?î¬zP—áÍ?Û€Òtî?Y&S.§9?W	­Gˆ?(?¤o*`Iîk?^¤!É.?ï|Î"?½OqW~?1jj ¼D?.U½.Š"? –ћû?½QL'™Ž÷?ïÙWµ®'?nÅýmYÞ?R‡׫Ê2?OŒYv§?mG70ê?iÿDˆ?ï,¨6ŒÑW?éõ¸º'Y?'Ž—ë>0ù?j z'`²?'#­<
]¬?|ʋ}¨G?ï¸É̬o?i'®²"7@?ErÊÄÆV?467O£?€vk5'çÙ?h¨H:®¶AGN3FGL J0151.6+2205@aœ~`Ï6ÀCU˟¦#À9½#nšÀ;º£ø'Ä?áÄDã‰Ò§@š§_Tú-@;[áF׿æÝÓG7p¿çݶÂs¿æœÛàæà¿ïÿ}¿|AGNfsrq?琉Íiù?ƒ'Ÿ6yA?v½w£/Y‡?zdʗ)Þ?u|!µ­®?tPñ¥˜W/?ès¿¹O'Â?¿C§°Ä¿ž?¸hýÙ)êo?²Í•&Î0?Áü'/xF@?µ¯\?í8¸¸îž"?œ e‡5—P?§·YÜn?'2[$œu?¤¼äRmY?ÒAaçT!?å¤@'#Ç?³×°QÀ1Ì?Å!¯ài?­Ì.4yaô?ÄMåïÆ?¬ÒúÜ|-¨?ïޑN ¼?o୐ky?`bÝÆd?d
4<—½Ñ?am‹¢É%?``»þ¯Ê?ígÆmô6?§Ç=Ñ"Æ?¢q¾rÎ$?äî<ð1'?§…$9‡?~˱žû?î°öæYnd?‡'GÞї?™Š›¬0(?€LCçg?Vˆ-þ™b?vqà=¨:?ìžÓ`¬'?š¿aJ	óÑ?®‰ÃôÈ$®?'IÔމг?§‰ñ½w8?'.r‡› AGN3FGL J0152.2+3707@a
¢À8+À~à±À:>'d@ò9À;ârÚ/­¿Â©—âùùš@&¶£Ã@@vÀP½ˆ¿Þr²™3±ø¿ä®K×¼6t¿åˆMD+~¿å–IÕ$ùÎAGNbcu?ïå(w²,ý?f?†¤Þ"ö?Xu Ï<˜?`Ønê
¹?]–›¦ÑÈÛ?Yv¯Rt1L?î÷H¬Ÿ¹L?¡Àô
*/¼?,
uAŸ)?†ÓM m~v?˜€ã©Øâø?öµïߣ?î@úä2Ù?'ûØòØ¡®?–Ä^ï?"nB?¢ý¥? ŽB3½Wö?ˆkícñ-?î4­`?•5w,W-?Ô…†'#?rÜO@õ5?¨@Fø:?"¥Ó—Iæ²?ïæH/³e·?¡u&dò¾?dà%°÷?¡wÆÈí=\?FÛÁ&™+C?B)ëÁ
?ﱪvØñÁ?"Ô­4䵸?d¼þFlÿ?d
Ó@¢é?|ÌE‰@'?ƒþ%Ú
?ïYU"í?|q{Þא?ƒ×ˆŸ™¶g?vͶ ÌË?…äâ:\v?l—
Å/àq?ċW?s²{T—?e40	»F?O‡"Àƒ´?'Ï/:Cµo?q6h4X`AGN3FGL J0152.6+0148@co€UûµÀLÃ)ßÍZ'À9qè
šó6À;rÔ#&v?'¤ŠŠô?v@'˜ª†Pç?þ/žÉ.]¿ã}ûüþ¿ÎU²;Hwà¿æ1ð\7Ó¿—TŒQæ_AGNbll?ïÙtLÐ_¡?lÏãÒ;Ü?TùÉ^F
?RKU^@?lΦøñÿ?gTIS"%^?(,;j?‰?ÛbÍç?e Û ¯Í`?sʵ]ÖÞ?…'?ãz'?ƒ.÷?î`â•Ù=?"Âà ûHò?—²²K?$?‰îVOæôÌ?œIQ\Ýß@?†Ë8ú§¹]?îDÎ6ë_Æ?žÄ°ËCȝ?`ÕÜ}ˆX·?i'ӊöN?ª¥¾Êcb'?žŽ¤>?ïôNe,™U?QŒ!ƒ¬Ì?;d¾¼ÉP?7UjW£èø?PŠށw.?KÒɃVDÂ?ïÜù_tQ-?kýúiڎ}?Pc¥Z,À?P³'\?jÔ͞Å,¹?f-El "?ïZ²}&o?€¹íï«¢Ç?…uߝbe¡?zL̈́sêÎ?ƒÝ%¢­?kk"4?úîz?wõšHu?Cá#Ø<km?@·œP.Â?ˆ`¯D%t?vµ˜yCBâAGN3FGL J0152.8+7517@_¸Ôýó¶F@)ÈÒÀ+ԚÀ:–›¸WËÀ;±"Pª<?ï¤ãŠå‡ë@1­@˜?üS ?ïD¹®j"§?£«ÁlúÞ¿Òò-¬-}¿ÛZâÃÈÛëAGNbll?ïßw/L?qð˜hÊú?^kr»ó"q?bRá_'?aS'yÎ?càj0Š?ícÉ+`3¥?¼&%:™{^?—*ñkÍt? îcœßV?®-ô–%¬ô?·9X"…?íÙS —í?›­}¡øU? ÷5C=H^?'dàŠCæ?¡s˜´.Ì?'BmŠ]kµ?ìl›?®ÚøRšS?¨ã"Ûáì?¢¸,zÞø±?°( ºÈƒá?¥I1D˜ Î?ïÉ^è1›ó?¥bæ5Eà?n×æ_ˆº?—€MuÝ/?h™?Þeœ)?–«&¶'py?ï&ëvR?¢ñ-™à5?¿ð¦ÞÏ?ˆjӅ!u?'B˜é¶á€?œ«zÒ?îûY6@ó?‹™"ˆŠ2?¾É¢9.?'§æ¡?¬ eîIß?/A
GÛq?¡]›?'Ô·eUœ?›¤Ù.S&M?…ÊSD÷?Gå]A˜‰?ˆ૓ü~AGN3FGL J0153.4+7114@_ûÞ¨—c@!òU¿û?À:Fó½Ò^À;¢nfåè'À›	º"å%@ÎkéG'?ù~àZÉ$?ÙhS.-î¿åVüæ¿Í$Àdð¬¿Ð¡}ÇñØAGNbcu?ïÃVûJŸÈ?Q§֓?7Ô§µ)?69r²©i?|×7Åû2¢?€×µf²D>?ît°è¯p4?´³tìN÷?wÒf<fŒù?…ˆ‡:«Ô?¥º¤©ˆž ?³¥®°ì?îE§:RH?—x5{
ƒ?9!²øÓJ?~<Øçwôß?¦m]Q#»?"Fp€/`!?ïuáBœÿø?†ƒ^sò£É>þÌ¥·SŸ`?‹…K[Ï?'<$"ªÛG?†+°¦?ïð8éšQ¿?Z£­¨?.¡ÚB)K?*–2ïÕ'j?[¾8Tn8
?X°»4ü?ïÔ€$?'£æ_×[?]Q˜åCÛ?[=ì€	N?"Øñ¬Eþ?'¦Ì^ÈZ?ï-àgÖ X?†X*FL+?Ç@­¯z%?rwœLYþW?'`R³Ó—ò?'¬Výð?ïäÇeV?_J¹Ý¿âÑ>â_Üs~ƒ>ä&…Wã?k&:¨¥¬Ÿ?_BwøÙ;AGN3FGL J0154.0+0824@b‡…À3aVÀI® ö½À8)+rt'À;
ú滋\?ò…­¶Üöf@¯í|Å£c?ýÀ(~ú1	¿Ç'ދ'A¿ÞF²ZÊ¿Ó=ЊòaÝ¿á>qðˆ=ÒAGNbll?ïzºxXΛ?‹Eà¸P¹¸?o¿r«H
?hè;ÖÙ_¿?‰²7íA?ˆ\×1Ú·?î'û˜<Lb?¤ ¤Èô;?‡pÎ/‰–¨?Œ…X¦5:?¡íÅA? jXøåf?í@&
֝±?¢kõöt? 
8¼Tǒ?û»mkø¨?«óf•ev_?œM#Š£Ñd?äå°
Ê3j?´òø•ßm?¡Œ± =Ñ?™€0ž'\?Ô	¶Hb+?µjý¨Kˆö?ïÀôz¬*?~»vqJë?fÇìcÑÉ?gPŸV|Kq?t!þbÈE?wÁ—Ö-¾?ïpÚ&ìAÌ?™{–Ã3C?vJ‰f@ˆ?sØ}·Àd?ˆ¤tô:¿?‡Ä€Ýf÷&?îûý~ˆ?Šp6‹Y?™Ì¨bº?'X¾-²Ë±?Í Ìמ2?®¢óé?êlÄ¡°"?¤ƒœhg-È?¦«¿¨›?'‹ž¨Mñ¸?À¡ý¶y¤1?¢,èzÚ AGN3FGL J0154.9+4433@`Õø@À0Ý¿Sg†À:_`¸§|À;ÒËÖ,Çß¿÷1ϨÊ9@f.fš¾³@w€ KÏâ¿ÞzùWf¼¿âÕ
Ý}
¿è"õïʗ'¿¸b
CVÅAGNbll?ïô'«ÚR¶?SÖA6ÌZå?.h‡(›H—?0—ž"…ˆ
?Sã—t'Wh?QíÁ®÷ó?ïˆð¿ù³=?ŠQ?ùð:s?k)N!Z÷}?uUʒUò—?†ù|n•¨×?ƒÅT"#B?îÔ﫞ÿµ?‹Û±	îÛ?‰ÙΌY?p1±®Y?•¤Ùþ4?€ÅB[–?ïޙfÕj?nZ÷P»¦>ü}â rø'?Óæ3Az6?p–Γï\)?mþì/lÂà?ïûÔ¥ðPF?=}ã>µÆs?BœkàÀ¡?¾#úe
±?:J)(?tå?9ƒ.ãVk?ï׍'ßî¾?q% 'i 4?TÐCFŽ‹?Wh+ëœÂØ?n
['Ã7?iàº%1ë?ï‰èì4"}?u®½'÷0õ?{Ëv²K-±?n¡ˆßÏâ?@+Ûïã?kÿBªN÷?ïúõþäù?AÅbbkÛ±>Ëá׸U.ˆ>ǁŸêRKº?D!Í+£ß?A¿ñ¼ˆAGN3FGL J0156.3+3913@a
Ô2TçÀ5î¬_nû`À9ƒL8½¶¯À;Ë+/X³À¸ûh¾@(³Ä"t@öA?»VÙ¿åŠXµ	ð¿è_Pé/6­¿à¯öäV	¿ïÿë‹åãAGNbcu?ï¦\Ü,™Å?¡'[§X?+ì;¬ü?1Ú×0%?¤?…üiQæE?¡‹
J!~ƒ?ï‰7Áã9Ì?"'	üz†Ñ?o…ÂSe?!?ïoì!?…Ðͧ,&?‹ðàeFØ?î=ôíïî?›¦;íÑ?'K¨v¶}œ?€´òô}b¦?¢úêÄ
ôP?š$8 x?ïåpNJºü?q.	Þ^?¥Â	Ô?Qª
Ÿ‹?jD¡ûÖæ,?q['ö°×"?ï›K~Q? ÜƒhÉ¥Í?0¶5Vswˆ?6†çÏÍi?}¦öþl/? Æ5×Bë?ï×ìâ°¨™?p_µÚg®?UÍ(ô2E?RçÓ0¥?mŽ¶ó6åæ?jàFÜÈ?b?îÌÙ¨[?"n6"f©Ø?Œ).…K^?{	¸QFïÖ?˜P3·!Ö?'u¤uTe¿?ïü+¿BíÞ?C»h
Õ?é>­þ3€Û©ï>¿d1›y†_?>"!1¬M?C¹Ú¨LAGN3FGL J0156.9-4742@q6`ÀiçûÀPp×?íUÙÀ:õ©ŽÚ"÷À<&¬k-v¿ö¹Ô,g'@†Q
^¨­@¥ßx "?ü­–‰¿ïiŒFR}Y?ä(_ÂÞ6'¿¢·JüÊã¶AGNbcu?ïÙn©+?yÚ¶ŽT¿?Dë×N&^?o¹;ý/‹Ì?p´îÄ÷?r|§¯R±²?ï©?Iʁ÷?†^Û'ƒ?`˜ Þyøà?d[LñA?Šao¯Ü?ƒTz<ô]y?íµWiµÓ?›»Ð¦ :³?'´÷±'?‡·I´¨3?«Ð
"«,Æ?™y…a…)k?ïØE΍¹‰?v³<-=>̎¬üúâ>çzøTþì?sنÅߤ<?v°œŸ@ù?ï"Ú¼4àC?¹.¿®ß¯†?"jŒ]=j;?¹7ðÝüû?j{6¬Ž?x`¼pC?ïà÷é¨r?jx|­–w?OVqÃoëM?PdŠmՏ?g2y¬k¼½?cß¼û?î›I<èqL?•x/Œk¥ï?ˆ†k'??"t+•îàç? )æ­nn»?'Âe[G¦?ïû
ᖙ›?E=©
+Â>ÃOªûº…+>˪)•	?CÁ)‰Ò"?E3ìò½ÎôAGN3FGL J0157.0-5301@q¢ß?–ÀN°ŸõÔ-À9ž´À;(Âz?ò¦Ì,¾Ïß@Œ,ºÉ1?ý*
h¦?ÛM{'ƒ·¿¾x9cN¿Ì5¹åg¿æ WÊ}AGNbll?ï³»me?{–VçÂð?sùɾÓ"?q¦'ëƒ&?rvXm›ì?m#O³Å'?î6u?r0Ê?¦%²Ë|'8?Ê ã#¥?û§.4<?¤3[ýûœ? ':É5±?ì˒˜§ö?¥:_Nÿsf?ªîRÉõƒ°?˜þ('é!?¨Xƒ©âë?š‡Q©§?ëøQàÈW?®ê)˜ÄvV?§ùÃõ¿ˆŒ? V4
»É.?»Ë[wcÓ~?ªÆÁo÷^Ç?ïÚæ[û9®?khë|"hì?e0ÂÄ£ò?b%¾nýÇ?_ÑÂTIÀ€?X¥Ù‹—%?ïÙ DÙy?"saW•W?†óüä"¹?‡-z_}Ð?'JÍ|̹"?‡ìv¹¯?î©üäJJ…?"+ ©¾‹ß?™ôÖæˆ?ÕËSD‹?ËŒ'æuT?"N`§=?í¾õÙ^M?–'þa}ÿ?¤F†ÁýE?‹F@OR-?Ÿ"^üw¥Í?Œ ðï&AGN3FGL J0157.9-4615@q
?ÐÐhÀP²uÀjÀ9Áj©ÂÉÀ;çl¸ÿ?ðÎeä¶@H'"Í.Ç@˜[À6ã¿ÞôË·"ž¿çœû7昝¿æèf">®¿ïÿëÆj»"AGNfsrq?íñLD7?¸,Xá^"w?˜ønì:Þö?©ª®"Óa<?«"Iq®±?³	³Ýf3?ë0`ãùà?¼V	ªQ?°+¯e›«¼?­ê¹2@bÿ?¶QIy¿¶C?±Èé­/?ëÉ7~Ç[I?©ÌAY&b?³@Ìo	7?¢dÅ­láà?¬êï2ƒ
?š×T¾‡àk?ès¶dÅ@U?³­ó¬–?ÀMœÓs?¨uäÚEí[?»Ç³ã"1?­ó¹Õ–x?ìÏqF¶•?ÉVKóëÁý?±§Û:t?ÇðW|=¾? èÂC(k&?±A@Ž¦Ò?íÜÖ¿®E?¨óX¯J"? Åò×7/?ŸiõóÿÅ?¡mšƒÁ™}?˜¹ÏvBÞ?íë¦&Ÿ@?¨RóƒÇ?£²࿑ß?•K&ˆÄ£ø?›'5›dÂD?¨¸¼Ãß?í€Ã5ªÆ?›pÍP2ûÞ?ªþ‡Þ÷?Œ×ú¬ã?™ëZV«O?',Šò"9AGN3FGL J0158.6-3931@p,Î?þó'ÀQÔÀ_×,À9XŠÙã5ÅÀ;Ã¯Ù`?ÞÖæü£Õ@ë«/™Ì@.HÿxE·?q×U¼Ê÷
¿ávþOž¿âÅ
¬N¿Ù»+ÅUµAGNbll?ïùZB¨œ??!KªQ?-¨gÝWm¼?$á½!´û?C+¨O5.Æ?8é´Ã??ï€ñTk'?'$æiê½?mǹÖè'õ?ktÿã#?ˆQ¼o¹I®?‡?fzæÚ?ï9"qø§?ƒÁŗÚ?ƒÙ&ð.?tٽ݃ñÂ?Á½Eé?{±]Z?í~²Q
? Ð1D´q?qÝ"[´"?mλ[ؐG?²ìž™e? … %dhŠ?ïûÛ¨²¼*?2¥'Ëö¦?%1ïW|ß*?.b•ˆ‡?6‰ÁÜ,6?*;³¬ï"?ïÙyÊWÂ?nßbŒTR?RÚ.è©TÖ?QmY?g_?mŒ	?húWèG?樓ê½+M?o<'ZuÓ?t²Ù¼‹jd?d.‰B^É?x†°ù|—!?cÔ°‡Ï¬?ïnPó€Ý?³¸Út¦«?a¼ 3íe?R—Aèý'?ü¼¼yçy?~W
Ep¢AGN3FGL J0159.4+1046@b–¯ÀL‹ÊÀHT(?º*3À9MPíX]À;€¯°î¿Ð	'û%áÍ@Ê#EÕLM@èHÞ½¿æ=ô$™V¿á©'¯èˆ¿åãtó·¿ÇÃ\ôÖ3ÜAGNbll?ïô#þ.f?P!ÆN?:</6–»¡?8:¥Mm¤?Q(øS,²™?HúFÓÕG?ãç¬?Š·UH/9?ekÿ$´Oˆ?g….± ýY?‰~ÇJÅ?‡¡mô0[@?ï61dsi|?'êbHšY¥?ƒ¡´wÿ^?uRüà'~Ü?ŽÑòmɛ»?x§P-ÃFa?îêѬÒÓÄ?'MðQJñ!?D­ðNΫ?Ië Å?¡1´ã?'7"®<?ïùׯ `ë?@êÂM%¿?0_ŽÙzSl?,óìmq]"?@q|‹>&Ÿ?8_v†d˖?ïÜL"ƒ/J?kòŠ°¢fž?Pä‹s{δ?PŸÝ@8…}?kA%†™¯?f8
½+?ï©ëKhR?j€±®ë¾?rý¥ð-'Á?`ùsž†1?x´Ba)^?aZ\bñ'µ?ïÇXEnþ?jÛJ{ê«1?-©.²" ?'-ÄdÞì@?{ŠŠdGÕ8?jWÝ#iŒAGN3FGL J0159.8-2741@k`–óEÀR´›€#¦ÎÀ9þ¹=£ÏÀ;ضXí ?î!J˜]7@Â5'ÿùJ@JIÀ4¿ÓdTªô'@¿Ó§¨Ì£˜\¿á-=…œŒ"¿é~"لý<AGNbll?ï­òΊ?"¹ÖQ¿á?
…âö¹?'þóœäŒ?cóãT285?]Fÿ&¾ì?îš/ý&dv?ž­ëœVôj?ˆÊÑÑ '?‡8ötC§R? *K¼˜¬r?˜g'JØ?ìÓLƒÄί?©l1YþÉÖ?±®;"Öâý?¤É]öcÃ?žÝnã4.?'t•(EÄZ?ì¤õ‰?Àq?¥u¿[áWg?¢ñ0ª"ðô?'><´¥ß?±_»b¨Qÿ?¡cCùØ]J?ïßÉMU7.?s€³ˆºn?fwÅc=éM?qT þ'?S}Ú¥Q—?Oêâf½?ï|ÙU­lÆ?‡þÕLrè?x.Dý6­?w´ácËj?"²ˆ"Ç›"?}rC³@Ü*?î'Ð]Œ3f?˜âîS-š/? ÄÉ ¯rÖ?–@ÉáÅ^B?ˆ8ÄÅ¿<?€-D*­Ú?îÖìzj™?‹¿Ôô=É?•'~·$ È?xóƍÏÖ&?õþ=jì?"#D–˜ñAGN3FGL J0200.9-6635@rGÆŸ¸ÀHñ7À:/œÔ·|ÙÀ;ñò¤ÍªB¿ï)÷é00@î#Ž¥u@¥ Z¨î¿ãµ¹óA‰¿äÔÂâ4µa¿ç+À"‡b¿Þ(>Ã4G°AGNbcu?ïîüšoØU?bÍÔ~G?9H"v
šã?6@̞:…B?[´©ê›|	?a&ïMkEÜ?ïŠ~O€
?"ºwõ)ï/?fé¨-»¹ý?fÕrñ@f?‡¾¶`Y?þ|<§?îí´è²J?Št4ƒŠü'?‡³`m'¥k?t£	\°''?–o¿Ïÿû?"Ì–A˜…?ï§ÄXEM?}‹Z¤)Ø#?,ͬ‹Û¶5?/rEŠÎpÎ?…Ƙ17ü?}`0Mló³?ïùÕ®j-"?G†|«³ê‰?((álý­?'Œr¥–J¥?B¤|ÃNø1?D@žRE?ïÙTŸ`û:?jü'æžd?RVpªÛ?PØVE—pî?m€(S6+?džÀ®´ƒ?ïšî!Ü?p@Ü
»?t×úGmH¡?`-ѱýUc?}è´³,f?h¸lû!e(?ïñDgÁ?TP¼Dº%H?ÿb*`…ú?eñÜNt¨?]|/=<Ç?Tbe"F+AGN3FGL J0202.3+0851@bݍ`¦3ÀI/ÿ¢/À:€\GÿsÀ;ÕiŠÞô?ï+Í+þqÇ@
=`'@as\f³?ïÿ—›UÊ¿àZ¦íÈ£{¿à¯€`¸}¿éo~ýOæ6AGNfsrq?î´2ö]¦
?´ƒo)¼8–? ËˆLD…?²ÖM丝?ŠCò:s?ŠÉ\s×Û?ë›ÿªUæ?¹Þ+èÕÜ?¨¢ 0:&?©@¤"!?¶Ö‡éFiÂ?²K¦üS")?é›RmyïÊ?²ÚÉx3É?À4JŠgÍo?¯YÓ¬¡|?²¼×ÎÚS?¥1œ=	Œ?å	ú-"I	?»2‹}?IJÃ4%T+?³E.''0?Ç%T‰‡±?´›×®Êz¯?ï×öé?°8u í«'?'ö7Öæ>(?ªÄ¬Éþ4?'Ý'ÑÙ?w,Ó¡?îA>•£?¯÷`ƪ£÷?Ô¥6T?¦<®]? Ñ›S-#¥?›{3ñ¼I?íà۞L?¢­€áyȒ?®G‰ä<L"?5'n?¡štzš2Ã?'ÿ)¥?뀜ƒ¿ú?¥Ù¥Z;7?ºÿË+%âW? "5àZÞ?©è_èWs®?™5£Ë­°*AGN3FGL J0202.5+4206@aԀuÀ2Öÿ_ÇôÀ9臢 PØÀ;ӗù†i;Àת´*8@z*ßQ´©@4JŸá\Q¿æñO:þ¿æêPé|…ã¿Þ#q_Ïڅ¿åíTW°@AGNbll?ïçû@ÊíÇ?aËä»Ná?<xI¾z·+?4•áòÁ=?du¶ù[?`ÃÂ,áÜ?ïŠK_œ?3?'Á–ÊÁÞ?m%Æ`š
?w˜u.	»†?†#¶qXä?Œ=ʐÝ]i?îéN|ÃS?Št‡ÜðÀÏ?…>`u"â?vÅÙÿÀ^?˜0¦+œgµ?"œâˆÒ A?ï×C܁SZ?s2X­X>ñ®‹˜íŠÏ?Ñ,F2¤?tLcA)&P?s,LÄó"?ïø£»í'¦?G{yí7sb?(±X‰42?&±AÍOÞ?GDº‡z̀?D5
<ÂÈ?ïÔ å#–ï?qr+œ¶?V¯|örŠ?TÏáÖ¥™?p®R9»ê?jR1«"²ñ?ï'Ô}›6?|+Ë^-tè?vèã!AS?w·‹xíÈ2?€{ã±ÛÒ?n
Ë|aÂ?ïø¼ïz
?H·âäó²>¶1Çc¡Dê>ÏÞKÈfÇÀ?M)¡œù¤?HµúÄõòoAGN3FGL J0203.1-0227@drä¼®ÀMøK¹ëÀ:hØÿ
6»À;ðL'8¿ö+?(´Õ	@ُ'Î@€Ÿ¨Qm¿ãÝêŸÛÜ¿ãÂ73&¿ãJ<ɦ¿íǔdâ"AGNbcu?îMe9&?£µk€X_P?š9¯S^.±?—•uk¾ŸJ?"¼®¨'²"?šÅxÎ%šø?ïeXGÐà>?•œùÉ¥½ú?p]®ÒÕì+?x@|öŒk?Ž{²ÛT?Ì7WƒjE?ëh>)Žø?¦•Ã©Õè?µÚ[™\? @O*?­ÂécÐAÉ?—ög¡"®?îäþZA?˜ßyÓ^??`˜š…ò±°?gXÔÏÇöF?¢¼&qºÊš?—ÞØ¥äy¾?ïNðŒ€½'?—3׉C?"ê &¹mÃ?†š>GGï?‡Y<Æ՝ô?ëylDÐ(?ïÕ#Õ¿‡?qkïQé£?U"gÌÊv?VaÇzèPy?p	UW˙?k?ˆÑ'Sò?í½"ÉXא?˜,cMfÁÿ?§Á
öÎßê?'VT¯á'Ý?˜ËPàh1?…)íL9¹?ïÂnÉ{"z?qlTÍÆÌ ?2`(Tco+?6»äªÿu?}¢˜Ùó¬V?q,¿ž_€AGN3FGL J0203.6+3043@a™Wÿ›V2À=¢ê šª;À8Ký¥²¬À;3˜ÿ?æ ?÷ÃkQݘL@†Êò9¼?ÿ?Ü+zÝ¿Ô\ãÐõPz¿ä+y@nì¿äAÜÕiº•¿æ{¬F‰@AGNbll?ïò%pk¼«?TÖ±ˆàû?;©9e'Z?B	ðßJÊ?TÊÑ"†"?Pg÷s\®?ï"I-›n±?Ž~‰Ááì'?kv[7ôb?€®çËÀ°?"PÁ0]R?'Bo,-éq?í"/$|â?¡ŽT)¦?¡=QÿƒÇ?•…:\µG&?¥½ºÅ•?˜ØóF?G?ïæTT.ð?oEHécÀt?œ´ÌυW?)ÌËGü?hÖÆ-õÔQ?o	¬Ò?ïùàÃÇ?C!¶08Ý-?3ébd?ùª?6<ƒZKå;?=}ÊZՂ?6ôìC]a£?ïק5°ÞQ?nú»¦iu·?Ub1•O»0?RëDq
´?m§±Ž¹5?gß~wù?îŽýã‰ìl?–ËpÄÝ?—Â]§é?Á~¨(P?—7ú¢†?=J%w­?ïûˆº‰º?Hd« ×? ø%¸ª?I‡u‰®??wZðSÂE?FóØC¥ç*AGN3FGL J0204.0+7234@`î¿eÛý@$ô "AÀ9-¯d9ÖÀ;aâÔvz¿ºýŠ*¡ûN@,F|ç_@ÅÈÿ¿F¿ÙnQÂ?€¿è‹ÌŒ¢å¿Ü©ÁÕwì ¿âê%Š(8AGNbll?ï?­»K?›29B~Æ(?xáxì«…?y¸ßÁÜWÔ?'çf?—½"Ó¦?îWÚ1D?³úHž{ìæ?ˆb§À¨ñ?Ž¥ŽÙ´?©"sÒȀ?±ýðÖV?íi€ÊÄ? ÝÜFjÝ?™7D:&g?†Žc/¥4-?¬ÌUÿG·?œ…¾4Gt"?ìß«€Úö?žç—Ÿ¤?v­ü>ŠÃS?n ò³üW?·—ù½K\?ž#ŽÜúè?ï߇+²Ù?v²µ"9À«?WÇXM¯ÅZ?`Ù½°Ù?d•=ð͜N?pf³nÔw?ït
)^­?–ßtÀaÔ?r'«i÷}?uhx‰†€}?‰ñáÚ%$þ?'ôÍ¢È?ï*WX›;t?‡HOá%­?"¢^¿G
þ?vê°º&êÁ?c啌ó?ÔÇ*°?ï39gCŸ×?zþ\4ø¾?eÍü"Öé¹?O߀	ت.?–ߎa³ø?z9ƒtã-—AGN3FGL J0204.2+2420@aí" ³Ô®ÀAΓ [TºÀ:ÑÊbAÀ;șÌÅ@¿Ê/'Šxá¶@
Óú=ž?ü­ŠÒS?ÕÛç·èË¿Ú."f\‰¿âÛ@°…€?´ïA8P÷AGNbcu?ïÌtÖÒÆG?€&vó?8ʘ)Ç[?0él.>9F?x8ë(4?€
cæèUŒ?ïqÑm_C?‹2åãýž"?g²€l‹<^?s
/×ÒN?‰¶ë'þ??†l¹Ój?ºÎ·L?‹¸nü?Dýʖr»?y"Äù‹F?ž&jÔ³kÀ?"¢+wë?ïmÇٝì?'Ð}"&ÿM?MV¤/×T?Zž|Žc3?ž'áí¯ì?'€JÐú'%?ïð>ÈMó9?`4ô?‹½Ú?%>"ÛxRc?²¼7Að'?\ڜ¿ûð\?_¸ÐÉ` œ?ïؙåèA?kpP‰S%?RtJ÷֚?MZô	S1?n,»}Œ=?gxaÑÜJ&?ï_î0Z÷Ù?vãóç7A?€k3aw°c?ms["¿?‡™@›
G?k"^œŠ2?ïÔ}Q©.Ò?iCï|zÓô?0GƒÔdC?2x'F¤?t¼æƸ&ž?h"4§³×îAGN3FGL J0204.8+3212@aü–þµÀ<%»À5ÖÀ9F	ç	ŽõÀ;åŒ·3?ÞÜ~¸@!↝h†@Ž—?w9G¿èð+Ña~m¿èz—U'пïÿì%úÝÏ?ïùqæ¢5õAGNfsrq?ïâÒGµ÷?—"$Wò1?h-½8aÐ?—‡×q¸Ì\?Cÿ좳™?Kü@o<<?ïmžãý¸I?˜Bá•Ërž?nÆÚ%@"z?vÏB ޘ?Œæ|ÁDú?•ÍNš\?îšxº"~]?'"à·Ö¿—?Œöxª§,+?~ý®¹]я?ž5¬ZžJ?ŽdÜ´²‹?ï‡g;Al?—˜U'QÓg?D‹…D┐?`PÒB:Á?ŒÝ€'ü5_?—{£Ü5o?ïb¹ÓBT0?Àg_¹è³L?"?ƺE(?ÀiÐ1?:?¸'¿ÌŠ??X4vãŒÜ?ïÌ)¸¤æn?Št,"°R?a¥êÏ ú?B'ÈëôŠ?q¡¯æ(¾?u
Ï,ý}?ïRNڌ0®?†x¹û
ýÅ?~ôýïÍè?tzñ±rƒ?‹ñÊVQ¥¢?ƒe*ãZ?ïô/N?p6ªŒµl?ŽbÍL½?4>·MÎå•?V˜zÅÄ?p£¸¾çIAGN3FGL J0205.0+1510@b€ºÃ.¾ÀF	՟Ú%{À9M­Ûoý¿À;¦G'ܾ¿ñv8;/ÖÝ@± üÏÊ@= v­†¿æ•'¢)`¿æzò@"‡Ë¿è*…ŽŽ'n¿æt=IaÕAGNbcu?ïúÌÏÑäå?AjlŠõP?&}àÐÞl?#Þ «Ÿí"?>Z¯*«æ?>Ø%þiŒ?ïK"ãª	?"Û0#›Ä?dÎ~Q¹a?eeaPÎ^Ó?‡(+ñës?ª¤>pK•?ïYt÷‰ö?…åëó&Õ?†[
`Ék?qŽ¦ihPÛ?"‡J«'¡Ç?€
Ì:—\Ô?ï~~Ý£?"aIœXG3?8]ы?@;¨!o¯ò?›5ZgÆ?"6¶œF®?ïý«)9	a?+짍5Eõ?•>ڛ,?©d-¾?)ы"ÎÊ?&
9RFî?ïÚ(e#ñ!?lC•ºgžŽ?QŸÅñ¦÷×?Q'ä-Nà?m·±Áo?ezs1zŸL?ï—MàÖ?lE²u‹Wï?vÚJ:?]î'Wû{?~rÞã~½?b!—ñÎ	ö?ïè?=ì'?_l 
eÚ?£}R`n%?(€_ãáÔ?gN4Ó0¾?_6jâ*cÍAGN3FGL J0205.2-1700@gB¨€QÉ÷ÀQ‰ÿ`2o¿À8ºyà–®-À;¹C'&?ëÉîóµ'>@F‡7¯D@c¿Âù¿æ»§[¬¬¤¿éËÄOr&¿ìÁ®Û¿ïþ%Õ|ž·AGNfsrq?ïó¿Bµ'?UMpÀµÒ?H6!»6þŒ?I`ƒî×Th?HÌÔÆÞ3T?JèÈiº-i?ïz;7ŽŒ ?U†!ö'˜?nGLîŽÊ#?€ß©''ó»?‰ß^䀷d?…¯ç"ì¶?îdO8*?"mµ}4e?üP¶
on?Šœ^‹t¿z?•yÈH!ºŒ?‡ŽÈSmÇ?ïqÃgÚk?Ò3vÌ{s?mîèÌÎÍs?seå¾/'ÿ?ŒkáˆBE?Z‰•=ßø?ï÷Êsü?HzÅä^…³?BÒ%´"ü?BKÛÙÑÙy?<¨ïC•A?6«Œ,	¡?ïÓ9ëU›_?qã(ê?X;ðkïZ?WCuž†I ?p];=štž?kiµ0eí?îö•5b–?‡»¸yïàA?":)$D5˜?vÏûwö?‰æm­Ž‹L?yY:ðË€?ïå_>Ëd?ts"ÞSäU?J:Wƒ4?CSÿÁB?dm&§'3?s€&¢÷Q^AGN3FGL J0205.5+6448@`VþKZ@£ÿywÀ7¡Û§[#<À;»·Ñ"?ùhÎÆ!7@ú˜Ê¼§;@¦Åæ(¾e¿àƒQé3$¿äŒ–EYÚ¿çè-µè&<¿í
9äI¸}PSRPSR?"E<šñû‰?…¥'õ­Ÿ?ìSóéWƒ0?ÀŸøeNZÎ?º×¹$y\?¿Ó{MåL\?IǸӲØ?a¾}
MÄ¥?é͈/Ӝ?¿*·›"¢´?È°Éx¦Ò4?¿!ÑÌeô§?Èaß=3"?¬óÝ7.±?ä˜rf
1B?³TØeÙº?Å<VætFW?¨|MÆkæ?Œ™[}¡Ñ?Œ¢‰:"|?íü¤Uà1?°f.MÁ
?³ÌïlRò=?­Î&À¾^?Ÿ2ûOÎÈ? Ó«¡ú~E?ë	
ß=Mú?Ê`OºÂ"?¿êê.²oÿ?Á¹ku]¾ç?aÁ=¯.r?tjQµ
ž?ê1
²ò—H?·Ö$3òé?ÆôÐ<ÿö×?·ÈòS˜N-?Ø`1ÑçÇX?±ÛáÚT?Ý´"' £?²+7å­@?ÃÖv$0?¥S'ÈJú?«w#ú?™à5~IÙ~?ëNhRq3k?°/nŸrs?·ÆçTÆ(?ª5hBŽ¹ÏPSR3FGL J0206.4-1150@eóWŸ#FVÀP¬Å@'HÀ9Z&d׍À;ÄAvÂÔü?²dŽPvv:@Gµpå›P@¦½M¿ãºÞì<²¿åRÙr2ދ¿ß¸ôäÕ}¿ëM‹,T­èAGNfsrq?ïöYºÍÞ?HÕ©¬bÊu?:$ÿÕ°^?5Ð7WèL?I†—Jã_û?C¿%¼|KI?Ök?‹yÁJ£?cø{'ßi?|1+0?'›Ùo/~A?'=Ò'và?îà"Uw?‰swíÉÞ?™w•Mw?}^00V?".ùÕ¨ðM?€ÅàÓ¡ž'?ïäݾrÓ?kŸmû§r?,Tט?)rHr}ù?j`ÞþWÓ3?jШ¦‰5ƒ?ïûMX£Z8?6s]ùÖl¸?1@ú™oO?(É44t<T?4T>Õg/‰?,:©¥r¼h?ïàrâÜ¿Å?nb‹ô½?O8ýûo?Q´Õ‹•{y?g¿û×%½?gŸ J-	Ë?ï}è­ËL<?vLÙлÏ?€­,@IJ
?nà‡d™Ð?±P¤"?i<`º9²?ïû'é~o?D'<e«±?¯3©ÜÈ:?Ӊ[J¥@?Bg»',Ä?DOüfAGN3FGL J0207.9-3846@o»'_ét£ÀQT_Ó¥.À:,x'¸ÔÈÀ;ü6'cDs¿ÔýÃw"@÷Îú¤vl@Zk@•ÇR¿ã[c$VeV¿é&çx¨:û¿ã¥¯½ƒ¿ì	i4àeAGNbcu?ïßñZ0g?j•jô_IÒ?Pðü]‰ò?R2²|óà?g–yÁœsè?eøñ•w–?ï+>§R]?šÑÉb"\´?x¿t‰'§?†7˜Ž%?"hM÷M·•?"[?îœêÔA-?"÷
›§™j?›hŽóZ•?†ëGU6å±?¢AêE®Ší?Œµ»¦CR?îÏ	èâ?Ÿ|B{¬/?{ÑÁ{"r?s±Åº%׈?¬O'^²¡?QHÚÕÈ ?ïñíâ??UL▖Ž?@ꡉQ×?@ù‡¯"x?S¯"ou¼?P/>^9.^?ïÃ,±œ?ƒßƂ8ˆ?`P
D9.?cD	ÚËCZ?vA÷¬¬iS?~%ډ;¼
?ïA|ïaD?ƒˆ€ŒÂ?TZ—f?yîÉ%h9c?‹F/ù½¨?t&'—Ï?ï ý²â"´?vyZV²+?\Ø\sƒZ?M«"æ©~†?"%‡ÅLøò?uf"éq•9AGN3FGL J0208.0-6838@rMÀÓgÀGy¾Ÿã_¶À:	~(úË
À;â½µÔì¿ÝÌǗ6pˆ@ÞXºla@]HÀŽ%¿ãâú˜ž¿çZ|Oz£¿â"Œ c¿æKõBÑz AGNbll?î¿%Ó?ªL‡¶êµ?j
ÕyÆJ?oŵ%?¦m33Xþç?©@Ì{}«¦?î£F€Sè?¬ÁÿËD
?†p^=Ì4?•ÀçNHÜj? /€eÿƒ?£óà÷vû|?íÀ(4ãž?2ɇÇ)ã?šc2–z?"w†z}&¡?°q2€ðó?—Ä0åÞ¾'?ì檛
{Ø?£-©_¾?ƒŸŒÌþ]*?{TŒcÃü?¶V¹§^X?¢=@¯Ï?ï­èÅM¹?—Õ‡9"i?VýÕëpÝ?kC•å…?´ԟ¸?•¤h$›7?ﬨ!Bt?‰ rõÀö?e¹>1_d½?s5Æ©õ?~ÏPY‹t?'ô"wÚï³?ï¢LàG?€ël:´Þy?"76‹Iû?o€Ó†n©_?'pqÆۋ?x˜¢=¢
ù?ïW‡OâbÙ?¼OÞXö?dË#%y*?RNdFŒ?'u´þsË?}ùìƒ_AAGN3FGL J0208.6+3522@a‡?'æGÀ8á݀y7$À:v¦—®ÝÎÀ;¾Â±(,¿¶ÄY'À@
F¹q?ûG޻⚿ïÿæƒhf?ïü™¬l¥¿ÆFóƒN¿Ý|æì™×éAGNbll?ïï6ÖD´?[Êm?Ž?&âû3§?!¬¹¸£p?^¶µ
>—?Zi/o2€™?îãzsíJ? ó
DÄ®…?ÊGbp\¼?QҎ/"?š«ÊÉáb?Ÿ$R­'n?îÎø½9Ô?†‹¸4®@A?‡×Ù¬jgä?q¨«æ'Y°?š5sÛ_†?ƒ2»™"«9?îòýr©b1?—S…ä"ª?"
¥?…TÀœsÛÈ?—žÙÙ×u"?"VÙ®ò>?ï÷œ½¡œÙ?E¯0·˜ò·?{Ñà?ã{šN?M©ZŸðò?Drœ_Jy?ïµãTΎ?@6,‰	L?dÿ@k¬?bÅñ€Ö?zÿî#úÌ?|1™³ûY¥?ïqL·ë>?rЊ#ó?zÅN¤¸ç?^æhºÕ"?†JWóú¼?ntGåћ?ïµßuú`·?pOp%öQ?k(Á'×¹?\AÐ<hp?w|9p"?jH·T™£AGN3FGL J0209.4-5229@qeˆ`VíÀN_JÞ™À8"Š¥àϹÀ;¤TÞ¿¸ýûh@ꨍþ0?üÊÈ`Ví?¯'®\¹Y¿á#}ë麿Ð*.QÌüH¿ÜàÏT!ÑrAGNbll?ïýy—½î°?-šGˆ?&·VÏ?`ßð0?1.j	íf?*"Ç }ï8?ï–0ãš.?ŒKÞµÙ?e{þJ‰?|0H×9)C?….¨&R¹±?ƒséž(z?ïã(ü?ïƒ`Å?'é—¡…jõ?wÓ¿=k¾?–.ÏVß·?ŠwªRñ¶Þ?íd¿×hT?ž0yé}?DìÎ#&ß2?E­`ÓÞ?´µpdÁö…?êàێú?ïþUëfbW?ú‰ր¹?Ô¡cz)÷?œ,Ñã?$l!Ôúa?w/å§cð?ïÚ~ÔÏÙ$?l‹I!N‡?REkCÖÅ?Pè;®P¿?l^uVCXš?f'ßÊ
9½?ï‰[ Àr?}]àW,…o?vã1T—,?eb
è5à?'7Ÿžï?y³ô,ÅØR?ï, ƒ>t–?€Z	*¶	?>ܼÏî±?1q¾IòÃÂ?š|Ÿ_?€A^˯AGN3FGL J0209.5+4449@a&uûmÊÀ/Â\ÀË6ËÀ:BÖ?<VÀ;ÒØ|-x¿ä©gög¡@Ø j™&?ÿ'DÁ%#ѿ߃õK$¿éw";ueÌ¿Õ²«·1Æ¿Å͚xÍØLAGNbll?ïû"ç$?=–ëùâ̍?
Óâ+¥"?*sŠƒ2?@6'kk?<Tz v?ï}òuö?Š5oDþ¯?mtìtà?p±J-a0?‰\f~&u?†g¡ÏÉ?ïð¸Ü¢O?ƒu2Ëɇ?#߰坢?n±K5Œ?›?"Ïù
X¿E?}–R'?ï¢66¦c?|Òö!³C?ÐÎOùŠF?%°ÍÛÑèi?‡LPÕIaã?|¯gb@;?ïýNäƒf–?(í4»v`?<XUET?ôƒCËâE?2ÁZ'|)K?&Ñ>@,Ü??ïÓhSÒ?r$M`´·^?WCKUÕ#Ò?SºùQîë?p¤ùTâ!?nˆÞáüL«?á‰9?mA¥ª"?s'óre
?ZáúÄ÷RG?€‰Ž%ös_?gÀ»—Œ?ïñ²£‹È?P Æ
Ñ?þIÐ j—?§=M!v?[ÒÇÚìív?O·é7Ž‹ªAGN3FGL J0210.7-5101@qAÉ 'RTÀNâD?Êñ*À7²¢
¢À;5ʎ.+Œ?øêò4:o=@úJ´Y9@»zú;¿ât}ŸÔÆ¿ãÛb¥þ¤¿æéãC!¿èDUºœž‡AGNBCU?ïîã5wŽµ?Z²É	…'?GFhI)´»?I¾þ?V–`ŋ¼—?S™ÖÚZ"?ï§:íºÐ?ƒé¹ÅÀµ?a ÕÎî}?dp%ϖÚ?éFôF6?€«۝Þ?îÕþq,
?†æ(ù?£zrÉÝ?˜´k×êb4?—pZ¡…M?ð%¯v?ïìSAèÐ?o*;ºV­«?,²Zvq?>no3¬Õ¥?bëXv4Iê?né6UÍ ?ïܛ7/"?¬	ÅáØ?DÕ40ž¥‹?I†df9£m?n/{ûôa¢?¬
‹DFtç?ïãOtÿ¨º?küâxœP?Kf@éŽ?Oè(Ålu?eÖúÐ!µA?ft¿&n?îÉATõP?•(‰wg´}?˜ÅbOtj2?"ÏÜ­³?Œ$ôY˜G–?"ÁmJû	?ïüÛÕ ¨N?F'E…È?ä4:Âç?g>igÊ?6¤Î‰˜ê?F2­ÿÖ¤AGN3FGL J0211.2+1051@c}sÉÀG®ÀGƒLÀ7Ƨf
öÔÀ:ì)é•ö?øf)Kf†@4ïY¿Ž÷?ÿU¥`ÍX¿Û\™Õ9éí¿ä1øh1οà÷[s:¬œ¿æ.â톼ÙAGNBLL?ïë÷Úívæ?[ñ¼óGT7?"ÅpGEÐÎ?#D¯Gº…?bÛÎò´t?Zý֕…†:?ïŠíÆ[]c?…­dìW›a?e¥¤ÿ½1?gÍXNAs?‡ÛL»q:?'	6lD&?îh&…ƒj·?šÒPë?EïÊéøÌ?Š&ã‹Ù|.?¡ZŸÄ&,?•¨òƒéϪ?ïyÞÿ»rÃ?‹Ìò{Kê~?CÛÅ>£™.?Q™ªu.â3?%AÚ 2?‹EÝÇÖIÌ?ïùhóÎ2A?D:S'¾ú?Îú›ßfz?ÅÊâéâ ?FÂQ^×i?BG°,ù'?ïÕ[¯±¼"?qO3Г¶?TŒ­ç°h?Sbç}š­?p.üë—?kšXÈLl6?ïGZ…e7Æ?ˆðÏòÀ?"; Í3Í?‹™h&É?‰î=ÍÐ^Ñ?€¶v[À\ß?ïÝÏß%êË?j½"Ü3'6?BN'B­R?<ÕÑTH‹?mœ|P8'?iÅ­Ò>Y`AGN3FGL J0211.2-0649@e3<`ŸÀOI¥ÒÀ:wò
ÎõœÀ;ò¼.ÿ?ÒIWMöÁ@ÿsì@Ë·À A¿Óì¿þC¿àÆۘäà6¿ÓYú6+Ný¿î‹o5~"VAGNbcu?îÞªêÇ+?œ[xç?œ6•ýӋö?˜q d
¬Ü?Ð2ˆ?‹{?€8Iƒ
ßd?ê`Æ>hE?±©Æ(?³¸ÏÛ±'f?µ§nM`g?¹@þ1è"#?µk'·\‹?éXöøžd?¬Ôb$YÈì?Á^ÓPA?§£b¡.<?²|<;,—\?ôBxÂ#?éïnz‡Â?²¼>+>/+?®Í6@c/k?§6î	Б½?ÀŽø…&3à?«Çø_tE&?ïkºì®?"3#âÀüu?•Ü¡Ç‰˜¥?3׿›§?ƒ+ͽ¨aœ?}ô'îý?í°ãY£Ç?°'K·š}É?¢™wÝy?¥"™'nÏW?¢XSEzÈ?œ¥'I"ò¼?ê_¡ge·?¨=¾–Î?ÀHã‰&Úµ?¤'ë¸^?¨ìGǁî´?˜<"!f˜?íæ§Å4È?•p|æé*?¡*t³0C•?ž9>m­? kûG=ê?ˆn…E"œAGN3FGL J0211.7+5402@`Ԙ€"åÖÀô'€—†À9¶^®@¦À;DDЩ*¿ü^øáӚ@
»Õtç·@‡¼à²^¿æyüàÎü¿é´¡¿¥>`¿ædŽŽ½ad¿çŒ
IYAGNbcu?í#0žA?²âÜí¹þÕ?'iË×÷?í
è5èÖ?´™]oØç?²-Üá[¾Ü?í™m7Í?¹P•åµ?Ym™éÿ?¤s.I4>…?®<eЮ¢?²MK«Å®/?ë`yæ²h?¨®«§ø§Ó?¦²°µÍ©W?''ó$T_?¹¢ØmÐú?£¥~Ŧêo?ìªD¡'?­(ȋŸ…í?XãWpÚF?_Ëð¥o?ºJMš×K?­´£ž×?ïÁáG"O?œI©¯Jâ¦?lxÏ:3"F?l—\Š:ó?™8©èç͔?šsʬ?ï4èŽc?§<—7¤
?rg£Éù?åÿù:Ê?"öi*m°?£.ŽËÄÀã?î«÷VR
þ?Œ52ÏZ?cÄè«9O?}ß?šPNË4ß?'ÿ£ß?ïü'|?ŒoM{ïö¯?0U!A»`l?3Cž˜#î¥?Ý«í.A1?ŒTl'–SAGN3FGL J0212.8-3504@nOЀ¶sÅÀQ¹¸!ïÀ:f°8AÀ;êTà,%"¿é#äV‰Ø@rå$ÝZ@ã矋öï¿Ë—pe~ñ¿è½VÃcË	¿Í'$[:¿ßdGKݽÐAGNbll?ïù\ªó+?FûFmÍ?hJ½`Àb?,§Úñ?H½ƒž¯Y±?E[©õV®Ü?ïš×ˆ×Cb?…\8|/?cPkâ?g\«Ç+?"‡Iºýû?œÇ½–"s?ï1ìÐçþ?"!Á†Ÿ?"DÆ܅jû?rŽMÉT!á?"^ôàš¾?††¶È¿?ïf8ôN'?‡¾-¤Ä?"¬øm?(äÍ6-?"þðû*?†ñ;º–>?ïü5s¼»?6O†1åÁO?@@ꞺÉ?¡«{–?9‡³¾þXQ?3™j­ÙU?ïÞn¥¥D?l}šøxÔ?PÑ»æ&?Pø_(UÈØ?iƒr2›â`?eëýxiÛ?ï"ï#ltP?nוޢ?v¤—ÿ,œÉ?c#æ·Iá?cÖRØK"?cÝ.µÝç?ïæ+O†rm?YÑJ 6:ª?ƒ]ñh…î?
"ÿ¦j?i@•¨bã?YnkØÀçAGN3FGL J0213.0+2245@bN¶¿DNÀB,Ì?ß À9L=Ÿ¿™À;ƒ*¯ÖòÀ¿ø9§v@ò3ä‰@Éè <öÖ¿ØɄ\µQu¿â\û"+7ß¿æ'Y=çtÌ¿Õ$olZ­\AGNbll?ïÒ1Žÿrù?roy2çv?`Ó"N±V?_ß²;Ö·´?lûq¸µä?jÊApMpý?ïu1>€2.?'0¨‹Ç@h?m‰\©†ô?€j'7J?‹QYA˜Y[?Š§¿cí5?íàþ)ˆ†ï?™Íbi™±?Ÿê#Èý¢g?*ÁÏE?¡û'ø¿Û?}'ÙºN¤?î—ˆZí?œT–ZIør?A5‰;V$>?Gç©ÐŸ;§?¦KQZ<l?œ3ífwº?ïêäT4y?asÀe7³?Lmù½$ñ?Hj‡œím?\ܶ‡5ž?[¼¹B\
?ïÒÎû6}Ò?v©.#Š7?UغH±b?`CÓ
¶{?q"bŠ¦º?pW—y"?ï!?-šöo?†÷Z÷T?Žü½"9|O?'aQ>Ú?ˆ³vûº?răÀzí$?ï®ß«Ä
ÿ?ué6FWb?úµÇÂÔ?¿K-Õâ?"&©‡†?uޏXª;AGN3FGL J0213.1-2720@kJµa
ÜÓÀQöÛÖÀÀ:ØU½¡¶ŸÀ<†Ï'yë¿íòcއñb@òSDÀ@µ­S·ã¿Ë—$¹¿¿éª"‡Ð³%¿Ýç'/xú¤¿º)¸[â»AGNbcu?ïÜé‡îvk?{gٚý?PCüß-/`?wê¸Sñª4?jôy|×5Ã?ihŠÈ;d?ï¢Q5t"‰?†ñõöó¯?b›¯?fæá‰éìw?'ÄÆåHkï?ƒ/h+Å!#?î!¶ÖbÅ?'†Üá>Š/?•©}7DW?†Ö«Ší5K?£T½Ú\%œ?Œz`I!ú?ïŽõWÊ0)?'^úÔ*`?ÝZ…se?#õIzE"×?Œï^Ða?'P|®uŒ?|áh?¹nßËÞär?"νêf"º?¹w"úã?VQdyf?K¿Íóh~"?ïⅻì)ß?kóÁ¨fó?NÁF‰?Pº;Úßzž?eùӒ¥
à?eJm&i	P?ï?¡Ïý6?ã(‹é^?"íx0@Ï#?|Æ"àl??‹*@XPGB?qüñv[H?ïïҋÜY?Uњçuc?÷ $Äû?€og'³ô?_Ë/`ç0±?Tõ/mc­AGN3FGL J0214.4+5143@`øÈS'^À""Vßà¥ÈÀ:'º'GmÀ;²B@p…?Ýóõ°›¾¸@ӈþ–É@Uü?V,2¿ì=b\I4°¿íeÈ9ü6X?ä)¡¢¾Ë¿âp6,·ÄAGNbll?ïñD'ùcÑ?\°
§µ+?+êÍ×?;S,–çÓÔ?ZÙ,ïÒ?[äDø'{?í±Ù†ÄÌ?·UB–lW[?‰²òeu–(?"«d]‡?®uª÷Æè¶?´"Q¸
?îGZÿÍM?'@̏?lŠ?ƒép­KW?r†''éY?¡1.#¾põ?'#qÏD.*?îæ:Ö¸?¤ÈIج£
?QŠ96{?hŠª¾"P?¡Èjª}H?¤£Ž@ô1®?ïòw֝¨i?y®!'>!?CêҎbú˜?y‹‰.¿ˆ?QêU5 ?LGÁ!µ¢?ï8"}ÜàÒ?°00Š¼{?v~€4(Å?{šÒÑØ?"Mð7…ßE?˜s"‰LÕ?ïh­åMk?'--å]hÄ?t%˱›?aÜÕ'ÂT?‹Á¡AûðH?Ã`­3é?ïÉъ¡¯?|˜;»²?Y,ÏÎØ=`?d«ººÝ?tÌÇÐÿ®?vPdaHƒHAGN3FGL J0214.7-5823@q»O?Ù3ãÀKØ'tÀ:MvÁ'}À;øшp¿¼ƒõÃf@ÿ/[bQ@O@…Z¿çs»
²›¿è'Í–ð¿âµpŸÐ?s¿Þ*x™Ä·ªAGNbcu?ïûµˉ£?:5Dê¤Y?žl·ï½?Ԑ
ä±¥?;ìf€F¨?7·ñD{ ?ïA#"bV?µŸ|Û
?k8ÖBhG?|n‹[[Î?ˆá¢rn?‡|Éá'P;?î®þN`Fx?‹ÓŠw‡Ý?‰C>F¡Ió?q'P'¬ö¡?~—î¾?†BÔ_ö?ïOäUã?Žböÿ­?\¿¤Z'À¸?^"…wWC?›Š	1@º'?‡ÕšþRê?ïýÈs'@?'q%WíJx?˜÷ý~³?SîÄ_?+ت5°ß6?#æ¼GÆc?ïÚ6¢?pi¶1Ù¢?RA€"—&¥?TY¥ßŠV?l©3þÿ¶Ä?ia;×aP?ï9ï÷•?qƒ'0EÃ[?vÚçMqÄß?Y~Yâsw?"D_ývM?lËì9‰?ï×sšèŠT?gw»!Ðq‰?EÏj4j Ä?:8æ™Ðï?qŒE#oΞ?eøû+ÀZFAGN3FGL J0216.1-7016@rO}ŸÓo~ÀF—€"ØÀ:)ݨ½#À;äsùÍ¿å²Åz'ƒ@8"IÖã§@…A¯ó£¿æä""Ðÿ%¿ç­ëè	Øá¿ç:dUr«Í¿ÎaßÆ$@AGNbcu?ïò²/ù©
?cqa~	š,?:­Ê¼Å?DmÜ嬽?Sð-¶,Þl?_½–¦°z?ïRÍ@?Œxƒ-'?g"Î,}Q?o[4ƒB±?‰â™Àu?†âڅf­?î  ›/_®?ŠÚ£v¨ƒ
?ŒÐ׉ÄXm?u¤z?ƒ€ÌšØ?…'2"P²¬?ïZ›ñb®?‡ŒJ¯þ?>qޙÇʁ?DY%ÂÁþM?"-åÚ~Œ?‡N3ï?ïöß9$ӎ?yõG*°\?4k¤tT?^‹&Ӗ"?JMå]…Z?rÝv­LO?ï֊¿ûÇÑ?qrÙ%r˜µ?SÒ%»>"?WÁ0–[°°?oŒ-c#/—?i~¹ÌCÒ?ïrî>âhë?s² \—‰¸?|Ì­ú\ð?dp)Óú?"ÞÖ^Ԟ?lë¸\<ÀÊ?ïæ7o¶yØ?aT–
;?«»›Ô1È?MɯÊVo?hë2L[2ä?aKFŠ"<AGN3FGL J0216.6-1019@f"ž²gÇÀO闟ÄVÀ:.\|ÙÀ;â$¯â±;?åÁ&5ò@…¿1¯{@¡NÿÂmx¿Ý¦ë®±¦"¿ååënù\ù¿åå'Íò‰¿ïÿÇ|ÆAGNbcu?ï÷§p¿'??G֘šIVc?<$ç÷jÏ?<¾Ÿ,·®z?COʇâ&?9ïÑLm?îÄѲ©yÐ?›DÈϺG?…<l®.E?†r«©/œ?œÇ"Uqqh?"qʓۖ?îb·ïd?"€ôXÃ?Ï? czË8¨1?¹ñXp?'â‹9ëš?'',¿N¨?íA,ò³~?¢"`›\x?›ÂG"'ig?=ō)?®
£am?žãVA'*?ïü+d‡¾ü?5½ãb&ñõ?,Yµ@F?,Ž®Îg?0šÛF¬í?%==¦ÈÒ?ï˜c`³°?¸*°Û
-?pý-FA?k­œ†å1?}P…ÏóS?yªïî=…?ï'ä5>?…©Soé«?"°l×µ,I?®ÓÆ£?ƒºmSß]ñ?q=0Mٍ?ïCTkÅ©v?EÿB/ÅS?‡TӖëip?n–ŒœKŸ?‡ÖiëÉ@?{§çiIrAGN3FGL J0217.0-6635@r%/€UûµÀH1" [TºÀ9 vö¢½À;±ù‰Ä9€¿Ùß-#û@…TøØþ?ÿ®Ó_Ž¿á
WÍ,ª¿âµ‹ñ¿×ôöí1Ç"¿â_O_¨uïAGNbll?ïù‡fÇ?@xWÏ	N?'—ιÇ?!Éἤ
?D0;'|ÿ?;E!mMì?ïsôn|_w?ŽçrÕIC?l ²}T{?},ϙ>Uª?‹ú·Á¢Í?†¤ î(c?ïR¦I;™o?~†ôŒ=•T?}E	f‰?p0"ä€u?Œ³é0m¡'?v'ïã!D?ïÏð»?‰	 —ÙˆÄ?H>2³6Û?ErÍ#=†?MÔkŸÛ?ˆÁȶ{"?ïü.'Rè?1¼õƒ4)?P
c×í=?‰˜JTè?77é—?ª%?-¸)Ó¥Íú?ïÕڑí?p.ÏàA?TA),×sú?Qõš¤?p/ÈoB÷'?jXîý¥çï?ï³~²†f?hüI4¤ê?ojMÎ*u?c<'Òè%?v¶ñ«ÂÓ²?X#¡SM?ïÌ;}'?e®çà'¶;?7Ãýkf
j?+'7šÜ¸?xu¢UH²?e*}°¢AGN3FGL J0217.1-0833@eÎWà&EåÀOB:`NqÀ:^XƒNÔyÀ;åú÷''ý?çNáAsì@
F`·{@£, šTU¿ß}Z"õ?Þ¿ãl³vS]¿ç‹MF¿éùWÿ½²JAGNfsrq?îÙÆónø?œ	è
A?"ˆ¾Û• ?•ÙþÚ(9Œ?'>b³ Î9?‹w	ߘO™?í
q?³³vˆ17<?¡ê‹ëÚNÙ?¤©…·îT?®ÓÕ2Tš?ªU›íA?ì
³|'Œ?¢:XŠhuÌ?­™ˆ™"0?˜=éõ›…Õ?°Ý›Õr³ˆ?—<Áƒ@ÝX?æ…\ï«ZH?± b_Ág±?Á¶íû¤.Q?«q~¤˜?Ä3žE®h'?«MÇ7{[/?ï®uî×Ü?h ¹R®c?p¯Å$Ýé?o¦´™¬Y?xc"rôO?uVá,8Ù?ï	U´ðë™?œÕVfǓ?‰Q>(]*ù?y¼œpÀ?',ªRÛai?Žÿk%U¢?îž*'Ч£?ˆö‡2d?––[<4æF?€¼¤zb
¦?•¤RdŽ»h?|²}ƒRù?ì›L¸÷?—æh¡¡rM?°Á(¡+U¼?'8Tzî˜+?¤Èã8h	%?–}18o#AGN3FGL J0217.2+0837@c"4 -œñÀHQö¬m²À8Ï}š_'7À;X}ÞR0N?җæEï£f@&âÙ(¦@ÍnB¿âSï¥X®\¿â›^HhW¿Ûx½­mc¿æáT~\|XAGNbll?ïýa*E™?*¤Bað?I(alEû?±É½ŒA?1í‡ÚÊ`ý?(d…¸8?B?ïK¯ÍJ?Š†:ÓKÓ#?h™#¬cM?{å¿—?††ËLZ—?V†—jµ?ïAqS[?~q ±ìr?€¯¡¯Yù?oéPTðâ?Žô-‡ú?4?wsæ|'NÓ?ï'LÙLŒö?€ð Xùâù?8i[‡‰´?CÁ7EUð?Š©~În
ë?€¤#É#n?ïþ¹ÖRƒ?Ÿ#"Z«?ú´Ç`>òGOá
ë*? ]ڜðý?Þ@fæ?ï×Id;؍?p'EÕKET?SXµT\aù?S0NÍ#¦ý?o
A&WÙä?iòŽ ?漢öÕ¤?iÔìr?q¥‡"ˆVK?bo·ñeç?yQªÿ\ëã?^?«ÄÅém?ïæ}'6"Þ?`…L·¾õ«?*¸70E?"ÒT0ß?gàã=¨0N?`$ºp½ûùAGN3FGL J0217.3+6209@`™ÀµgU?îÆ)ñkÀ8yÛVÓKlÀ:­´{/P@îcßxv@
Ç`|?üÌÄ>]ß?Ø%‡P8I¿çQk"ôÝÉ¿î݆þâHµ¿æËW?4¦ÙAGNbcu?ԇA­h?"s#*z?ӒTØì¸?Îâ-ؼ€`?嶖ï4§?Ï1Ó.29Û?[{lÁÎ?~(ŒNÌþ‹?áüõþ¹^?È9hù¶Y?ÛꘘEdA?ȃYw{É?É[£´ûtÖ?°5:kÙq?Ó¾La…V?²®:4ùÏ?ߓâ
 À??¹>*Nx­?Žc¡ÝWUõ?Ž~橱ƒŠ?è%|Ýæ?ÅÆoTew?̓…ˆ7	?Ãôßc?ˆ·ÂR	2?¹™";5á?á0ÌÏãñ?Ð"*ê0Ø1?ÜبM;?ÐäØÃaO?ayñU¾³?}Uð‡ôùå?ãŽÓ&
A?Áñ©·/<ë?Ø¿eÑ@$?Áڂ&$EÉ?Ï>êÒØeÃ?°ùN/è
?×½¢[ù¿¹?²ê'^Lc?Ø¢è:š
e?µ§©h?"Zܹa²Ž?ˆžFN.fd?ê}"üÄ??´U"R<>É?Ã~xL†°?²"ÈíwŽMIXED3FGL J0217.5+7349@`§Ÿì™ò@'ïÆ¡9¡À8šÞ>åÀ;_Ae%Ç?íxNµ¥@ì؏ù‡Á@BBàzS®¿çÉÍ#½R¿êv,g<$¿íNÀÉD">¿ïþ>F./
AGNfsrq?ïã:è¼Ë?péþµtæ?`dÒ1ü?diAL"†?YUeUxç?aî&b
#T?闭ìÀe¿?ÄÆÛöó?µžµöz"ä?±²=šäI ?½£Ú¡\í¨?¿V\Ë÷ª?í`z¾"ý?ž¹SÑÂ?¨Ý.½ÚJø?–-¬Ú•Â‡?¡%^)7?õ˜ϋß?å·9ˆjzÑ?»m§DÊW?ÊEͶùô?¹Â•ÚOõ¿?½º˜N¸AG?°ÉdîH—?ïèÍÄ÷ôÌ?´]êŠÜ?_&Bâ6A4?x4ØaM?N|g`âš÷?gµÁ^ؗ?íÛ>æ«×?¶xµy«Ÿ?¦.ûSéy:?§GÁ?èÝ«?©CPº<-V?¬rè§_/.?DIõ±?''=d|Š?žTÔrF?Œª°€+ƒ?'UIžß˜?'´†m4'?í.ò&¬×?Ÿî:Êp?«çF%ÍEÎ?–À‹³Ã_'?¡)—lÝg¾?•É£˜8*AGN3FGL J0217.8+0143@dE– hUTÀK5[ßú¦ûÀ7̄eTîoÀ;"‹›˜?ð­¬
µe¨@A*»?†©@‹ jC@¿Þ›Rú¬a¦¿ã¢
ã%§¿â˜rÉ\f¿åè×}æñÍAGNfsrq?ïúÆM_aî??eÒ	Yó'?Œq˜Á¨ç?äCZ"'?@õ=o(œ?;¶ÛÎÄØ?ï–ÒžŒ·M?Š¤ºK8?erz-/Š?sσ´Ÿ?"PxÃ?ƒí\ïC?îۃÄp1ì?'(áôÇÕ§?Š39à?/…¦2?—Œx]"¡'?Œ•­·ï×?ï‰iþêÐ?‰ª.돀r?A¤·©ª×?IÚ
}kÛË?Œ"†Ä_y?‰XƒÌ>6»?ïýÂJ_A&?#Êôùx'?SnF«æg?
$Õ¸ý½9?(1¤ÓÚ¹g?°,»?ïހŸ³Ë/?l¦;ÐP?P€Õ?Dˆû?Q/ߘ¸½[?i>õ×-³ø?fU«F¬ð?ïmõ÷ñò)?'.'ÀÄAí?|ÍF²P{—?rš'æº`?†Þ¦ëœ?|"­»Bî^?ïäO-mT?ilûöø•?67ögP|?8›9Պ"š?héÓä³9N?h±G
IaAGN3FGL J0218.1+4233@ap‰ßrïÀ1² Ñœ?À7Á¿ß~€9À;
~gäì@ˆĆØ@'Mp÷@ñ†‰qƒP¿ÞíC7À¿+¿ä_rÆ	ÿ¿æS=nj@¿ëöDyùã~PSRPSR?šý€ƒNýµ?šxÓ~×FY?î)ÃîVà7?¬gzÜh?ŸÊ©=õ†?£H8çË'?H²šG£?«£¤I?ìˆ~lu&Ñ?º¼¼¼çÚù?¹Ço'pA?·.&[˜ÞÝ?'IÖ)Ã?¬E$¯i?è!"q`¸?±=Aó`!?¹Ña È¦¼?£š•ôdz?£¦N8J?ˆ)˜
ënã?ì²Î¨ˆä"?¨ô‹t¬"?¶@¡'¼äK?¥à—ϧä? 1½»'¡?¢+ƒ'Ke'?íõQ'Ô9?¯	"CVÉ? y)*©sm?¢h ø9‹]?†¾²i?ŽÄNŒ–?웮o$q?¶ cDNJ?¸b4®–c?µšmôX?ΎҩŽ6î?°|)Yž4'?å¦BÄm$=?²IÁÃò­?µ°D†æ»@?¢+ä´oê¼?£îií"ó'?r«^·A?ì'Õûtªø?¡n¨Àƒ1[?±z,FÓü?šÄ¶Q+òPSR3FGL J0218.9+3642@a»»ÿŠ;À6ì¡`7x<À8Û§¦¢–˜À;Ccf×¥n?î3·#\m@‡¦ÞP­Â@› ¿ã…Ÿ cš&¿è…Ámüg¿æªÊo‹Q¿ïÿ؍ÚAGNbcu?ïä6<õK>?g!ÚCÏ)?XžÃ"Ì­?ZÎñhƒ9?^ô¨S?\{ÒvÁe®?ïN÷ðù
?À§¸[Ë?|Üì}™?9^}/Fè?–4©ùå¾ô?™lÓ6TÛ?î!×î¾å?•'Äž—¨?¡ÁbJøÌ°?GŸK±?˜B=—Y0E?†®™¯ˆ?îe)‡ã¹£?žaªZ€*è?˜ØòQ™?€s—'[t^?¥G1E[ú‰?œ<¸,€}?ïíý²Ùí®?m×t—\ç?WFµ©j&?kýó&N"?I{ÈgçÇ>?H™rý"?駱*Qüç?'_A÷uº?j/Úøí?e¢ìr'@J?€2)uª´?~÷LyÂ?îå%hf¾?‡Õ?¥q?–°7÷°S¯?'µø…mŽ?‰V5ð™Œ?qcC'Nå?mïd?}'žto?qÊi€Í?b%Z¦¢Z?ƒ·["P¯?zGú}"­6AGN3FGL J0219.0+2440@bbÇÿÞrÀAGñQçÀ:Oá4bÞÀ;ÀËÈÀΒ¿Úo3˜@^¸»F=?ý¶ô ü9w?ï¿J£!¿åo7ýr\¿Õ	äEöj'¿ÞšR=ÜÑÊAGNbcu?ïø–š
Ø¡?FµNvä?ãÕm[0?«…™Sà?JÂû¸@§?E³a–M´œ?ïmñ.ÎA?Q	á>ï‹?ižuã½BV?h)ËÄ!Í?Ž㦕ò?Œ±	Ò¤?ï*{°
Ûa?¡Z"Â*?':ƒÞk5¦?o‰j4l½?'"H~¼û?{òØ5S,?îyYüԅ?›¼·Ê¿Ô?N«
+ð€?P€§G­?§ïÂN§T"?šÂbüԛ[?ïü³Ké¯Ô?0‹Þ¢²Ê?K¹2?×l4ۘ?5Ò´nÀ?-ÇÏ¥ô"?ïÎÅÀ
"ú?rMnê	ÆÃ?WÀ;/5X?RsŸ†ÛãS?r­IÂ)z?oDˆ°¿+I?\wh?p‡-ÍjñÙ?v,$ßÿø¨?b¢VÖÀ?ù­8ƒ?gÀŒ;#û?ï´þ¸¶?râ6ù33?;j´§5o?0"a˜I¿¤?'#0%¡Q?rˆ:6ÅBAGN3FGL J0220.1+6202c@`¤4_½Œ?î(ê@6b#À8ò=)HÏÀ:FÁÅ1ÍØ?ôܽîbž±@>jÉÍhÿ@\[ÿÛ¿ß¹¿³4¿æà± ÷[í¿æé  0ø¿ïû†ô{gOTHERspp0?`U3§*Û?cœ%t"?¶+@Né`ñ?¸™Ôƒ€z?í*BÃ7çg?¸é…¦ÆÉk?š·ó,û=?¨þ`´ôß~?Ô¹Ïèh½6?ÃI§z'¶?äÍXrEÓ?ŵóÆ¥…$?º¦2ûÂÈ?¢jçít!?ѳßÿ75Õ?´*º›?ãÑI¬¤ì½?¶¡¾¶q‡%?¶×NW'=?­e»"pªœ?ÒùÀ|B¬ß?½"bwæ¹?ã¿$×ê{ù?Á£ÏNB"`?INHÝt?VE¤£-¯?°;BËQƒž?¸»ÍÑ"«?íòD¤IB?¸¯>	!¨!?®hX¿?ãž?¶7–Oè>¦?ÖÞ¿œžÃ?»"ïnÙÁ?âªs/óõ?Á¯|ö±ÞÆ?Ê%&,[õì?¬è…·zÛ?ÐÖÌêBÃ8?°vI&c¡?áOÿÇ é?´:|a¿&‹?¼h͉`;?²*x'ôý?ØÑË>AQ?³¥')#3?à
Á4×è?ºÛš×¥OTHER3FGL J0221.1+3556@aÓjßqêÿÀ7{/à˜[¬À7œë"aq4À;
.óŠ§¿ìc²‡QB"@Š|p>@A(ƒÓà¿ã'›ê'ì'¿å¿aC*»Ú¿áùx¸‰°¿ã£ˆŒ<JAGNFSRQ?ïù`ã‰k"?D‰¼"[R?æuPߑ¨?4l¸ÌÏü?G?£ÀwFŽ?CLA0ºU3?ï–Ø‹5Âs?"Ej–—s´?e²HÏî
'?fd;Xc ç?"ÝJû$CÄ?€Ãz84_½?îugÿ©Õ?˜gF?'•€+EÀ_?y£ì¤pœ§?¤ýÔà?–N0,þ?ïݟˆÏz…?pù'BÚ:Š>ö_"®€À?´o÷Øe[?qÜW~Ëô?pôÌDŠÚ?ïýiµ{L}?,%fß?HQŠµès?2¥58ÍÔ?0ÉHò‹¢¼?)±Žq¥~­?ïØý¨Ì?nS0A(?Sù¨ý¬"ü?R–gÚ]šÂ?m¬"ü‰™?hLSîœÝ?ï&kí
Û?'.vPbß?uU|Òó/?nïÒª?*Ï?•Ý<†™Õ?¦²ÚþÖÅ?ïù•Áƒÿ?H;Z->Ë 8@d34>Ño¦´Ì?IÚ
!åW?H42t{QDAGN3FGL J0222.1-1616@gÉ hUTÀP—L?ß À9|ÙGdCÀ;Ê+÷Տ?´Æ;'õÙ°@˜Hí¯›d@ÎñŸêìs¿ãìå5ú7ê¿èˆˆODa¿éënÆåµ°¿ß~ý<'h´AGNfsrq?ïùrÉ1rû?HGgQn—?*Ž]êÑÆ°?,Âðn˜?C'D'œ&?CÅIïP^n?ïc×Qb?‰X§°	}?gZ´ÕRãî?m·ÂŽ*[»?†Ð\ñ"ú›?…,6z÷~7?îþ\ø\%M?‡jƒ£Û^?…ÜýõÎH¯?xmR"#šX?•Eá÷Ücü?à€ŒAN?îڒ`üUb?–3։Hšw?dŽW0'i?a"¦ˆÁ`W?¡Ñ,	Â?•ÌDúvwW?ïü¿¡Éœt?6Jwý>ß?[¹Sm&?˜LNŠ?2¬!³'?2"ÇUþè?ïÚ¦$¹À?jw.g%ç?Qô$jS?O<" ;¢D?lCGù}?eßu£ÊÑ?Ƒt\?z0Ff0¦?xïÛâ?qÞ¸Õ?€Ó?e7†?p†4v>?ïÌæm\Ϻ?q'ž"8èÀ?F—,K?<)šWØw²?vÈè-ÿ¬C?pyª'ÌVAGN3FGL J0222.6+4301@a"Р+"À0ÄZ&–mÀ6]<¼HñÀ:
©yámn?ð‰•*6¢@$}õÏ$–?ýTÛ+µ:Š¿×>5фRÇ¿à¢L¢V£¿Üa|…Z¿ßCb¥ç…¶AGNBLL?챉HyҐ?½O®œ"¨?['—L!¨?a¯|pC(?º`ï®ú?¼¼IB¥RF?ï€öFT?Ó%&a/ô?l¸Ë‰á?oDè:Z%?ˆÊOŒ2½g?Œ÷"v«>?ç+"ô?²ºâà!£?™|9|òp«?".%ÁÖZ²?Ð*ÌÂL?±Uë"WE?ïC':½§Q?•È*UÝåË?æ}O‹¥[?å}ò˜ê?—ˆ2"˜Úx?•Ä ±?î&åH)ö…?´&òèÀHZ?TﱑҌÀ?\@7"\	?¬ê-ðNO?³æÒpÒZ?ïÖò'5q?qåië%Z?U]È'ð?Vi³7þ\?o Þ³†U?k!mc\Ó?èG^¿0µˆ?³Æ:M¹]?õO¹*ø_?"οþù"×?Ë#Û¼¸?²eŒ‡XŒ?ïÄaµ?xžøÀÓê­?áAxç?MHdÜ«Õ?}¢ñÃ7ˆê?xŽNEµý5AGN3FGL J0222.9-1117@f @FA-ÀO¦ÄŸ×¡<À:h|°TÇÀ;Í8Ëùh6?"z)@…Ë[ˆ'?ý'ýŸþbœ?ïàMH欿ڝû'¿ã5Ÿ°E>¿Àa
ÂAGNbll?ïë>(žs?]E¾íèY?0ŸÄÖ.?,ZÏæ+Â?b­Þ¾õpE?[@Eá-Ó?ï˜b"G?ˆá'K;Ö?cÊÕ_C5£?iâ=æ?…
2:¤¶?…(½1¥ô¯?î±ÿlÓÑ?Š€–
T´?ŽÀ…¢³÷þ?z‰¨*‰?š_Ï£ŠÁâ?ƒéž»^?îGÿÓµIM?¡ÚSÉ?a;í¤Ë?gG‹æmÔº?ªlQ	xrÚ? ÏÉ–è?ïöøï.e]?DE/LÄh? üdEÄ7z?›Ðºªù8?OÝ+$M*?BîRª5ì¨?ïÜôY¦?kˆ î¤ª?PåÁ6TE?PR€Ö1Ø?j™¼'Ç?eÞP«Z¶?ïi˜¨Ð;?w]֙a?Ñ*±WÆþ?n¥#æ?…×…·Ç?mÔ³¶OV°?ï°_,Ð'?vÿ>îŒ?E¾¢¤"?BjMÜ/C?'ŒJª^êò?v‹R9®ÛAGN3FGL J0223.3+6820@`hğס<@ãŸú[ÑÀ9¸À*'À;nºeÁû¸¿ûт"|ÿ@¼×ŒCp?þ£¿à€2ë¿èðÁFóµ¿Ø}j-4/v¿Ü¬è6ÆÌ¿¿ßšØŒ&GAGNbcu?ïÓƂ+w?t|±´žÿÉ?R®éÄø•š?P~•_¸?qqv›P?rU5È)?îs@õ=¯?±o"°
?wʙs³pÐ?|·Aî2ˆH?¥ÕˆÂ¬ò?°›DŽ5ë?î¦6;ä?'¹ïù}?‰ÌQGžº?w•èUè?žS,ñÒJ"?Ž?tùÀå}?òeQ'?€÷Vƒ=?\Xo8?$f_ÎÉ~À?‹ú®/É^?€éUÈsm?ïöM2Ò?T\ë{ì?4!Š›1?03)Á"€¶?Lºf܎Ê?QûÏP%d?T _?'±AÃÿ$·?`ý+™£5?cÑ™ûE?…§Ö[1x?»kÝeúš?ïzŠÅ7Ïr?yÇmôÓÖ?y ðŒ?c»bÎ͟-?"ŒÿÀ/©"?tVޔ»…r?ïäëδrR?\£çÓôÁV>ùûˆªÚS>ø2ã撾{?jà:~0PŽ?\1çÇôAGN3FGL J0223.5+6313@`¢Í œÃ@ye`,¨À9 @ŽÉ\À:ãPl)?ø‹×D;@uÊ\…!?þöx¥-K"¿ÚAøW
æ¿æ0NÃÌ6ê¿êö‡uœ©¿ã"øSIQAGNbcu?ÕhøŁ²{?Ƅ´"dŒz?×Yڇ™x?Ë#ܗßÉî?Ó=,³^´
?ÆÌn"C˜?ÑCW¶™?ӗ
I@L?Àù7	-?¹U'ÚÚíÒ?ãZ-á1*?Ò1ÚY8'¨?àj"æqâ?µ¯ï :±M?ǝg0³œ?¬7ÁXí…i?Ó]›¥n?¶Ã÷|}óÙ?Óô
ۂ>¬?¼ý³}#ò?Ðe™é0ìÃ?Ñ…ÐAª?Û¦X;Lԑ?À)«""[?ãìQªö?Ë8'8n}Ù?˼õ§•
v?ÅxÒj¬­Y?È;Y™Xµ?Â)Êòµ9?áùRfÕ?×ZÁ(:?ºN3ª&"¤?¸ò†÷ÔJ?×aW"ё-?Ó£B—K­ö?ç"ªÀÕÀ?±ˆ– ˜Ç?¿½o?[",?¦"iUfáL?ÁÑ%·t ç?¨\È-ÛÏW?Þ{õ¢a?¹Cö)0ˆ°?ÒêvI!K?ºzw·¾ë?Íùç((ú0?°iǐŸ`MIXED3FGL J0224.0+6235@`«¢_¦XÅ?ùáVèˆ?À9	"EœÂCÀ:lï­¢e?äc#c1}¦@tk0$µí@Íê€d?Øòtý¿çeg˜•›¿ëºÜ	€²¿âÑäÏ"£OTHERspp?âdeûåò–?Ϧ¯l>ˆ?߁Žcù?Ã\Q¼­'A?Ñgs%Uh×?˨B+#ö?ÐR뫛_þ?Ñ0²—cÖ¶?¼`ËV]¸?½Ö²ºãý?äJ‡1Pô©?Ч =À³m?ڃÍúì'?º×g–£V?ÆÀa̓¼?±kt=ûŸY?Ú¾KC?¸ZÖ1`?Í¥t4@Š›?»îjR†?·Z<7ž
?²,Ál˜ð×?å«[oß®H?ÀE?û¹?çÕw¨i?Ð
6q¿>?±Wh×æ΄?º\ý
qö?Êø÷UÀ™?Ìq(Gƒ˜?Ûåè^¸ƒ?ÓQ$Ë;}/?¹—ÊòKU?¸ér—C ?Ý´%0¼
ˆ?ÑVrIëÓÆ?åˆh	åÃ$?´ØřˆÄä?¼¦, ®?¦áR,'
Q?ˋIˆåc?²5½Eƒ?ص[`<År?¼˜&@Ë;?²†âp˜±w?¡™…2Ží?áTv—X?¼þ+\­³‹MIXED3FGL J0224.1-7941@ržq_ˆü"ÀBAÉ¿Ò‡À:ÏO^À;ÎïS	'¿õuŽ²Š×4@-#""±Ö@ÔÏbpã¿égØt~_µ¿ßÊ1%€±Û¿Ú÷sË:Ñ¿ç‰Äl'6AGNbcu?ïë>‰!?cs£×†GV?L)äÓÆ´?NW [ÀÊ#?[môð¤C?^
2ÜÓº?ïuäÂ,?…ÐÍɈ/ö?kd뚠Þ:?hßÄïÞG½?‹­"£:­%?'s³:†aú?L¹Ó1?'d¥˜–¿i?‹ªJÝB¨?z[Ä^Ú¤þ?›8PÿKû?Šµ5ý?ïpÞ½e&?…8ù@Ö?9ȯ³m?:%1–Æu?'•00õ@?"Ü2÷ÍL?ïù®Ëâ}?H;ªç+Èå?1Ál1>;Œ?1±ÄH"¼?@g*ýف?B{*¼7
·?ïÕG;—Ÿˆ?l'`›i¨?SåøÀ
9œ?O´6ª–T?pbä%ÙÙP?h
¡ðÞUˆ?ï‡õ;ù!â?uW¦vù
ú?x¡&5àÀ×?gde"^8F?²çw!?oþÈ+U(Þ?ïâù	ÓQ?]
±G'â=?oÃ_¾­o?Ӛ \?lSy«€"?\Û²ÆÞlAGN3FGL J0225.2-2602@jéÂ?«ºÀQA×,uªÀ9C[m TÀ;ÚºÌH¦?㧦¤¼YÚ@‹úÇ1€@NÌÀb†2¿æoû
¿è™›fÅ©9¿è<Éøj¿ïÿµððÌAGNbcu?ïûÑÒÆ?E«™õ ?#èEsY˜h?+Dé{à ?7}F¥Ô3Õ?Bé þ?lsÏ8?Š8gÅ¿›?e€eubž)?t4ìғ?">K‹2ê^?ƒm¥
Ã'ß?îî‹`Äw?ˆ'¤<;ÃÆ?"h$'
Ó?~μµ)Lg?Ž8OÍ~À©?}&aú‡?ï²$ȝ?å"Hæw?TX/ӝM?UÜüÓVB?€ðx,õG?'fÃMÞ?ïû¢¡'Eô?lêîB·¹V?*"SD,Î?S"‹èŸôÏ?5 Êïf'X?c*(³€ˆ?ïښØUc?m6~tG?SI–›¾/!?S1%:AÝU?kÀ\A@‡p?e©–¹­Ç·?ïKííc"?y?Òyb?‹tóš?q}!eο?ÆT3C.?kŽ–WŽ?ïñõmÕÆq?b‰øpxeÓ?7l»…?1i¹ï7«$?V9õ™È‡$?aºD¿äEAGN3FGL J0226.3+0941@cŤ p¸ÐÀGKÏ`%ÆÀ9'y…ýÛcÀ; dYEìs?êÐæ‹Kx@Aw÷ˆb@}±ÿlc¿"£úhóŒ¿èFwÓÌu¿ÓE
MXDÝ¿ëjò›Ø'
AGNfsrq?ïöTÊÔòX?K*;CÝ¿é?B½¼É#?AŽ~Š:Í?CïBpõ?@ Óó;?ïºQ?•YhÐC¼Ó?{6Z;ê?"$ +?—qÇ"¯*?TITóý\?ìþ!ƒˆ`6?¥O·œf?­æ{Sñ4Y? IÖ4jðÙ?¢7ltd¯A?•b¹¥ÖþO?íøÊK_œ?¢KÇ7cMë?~B1Üþ"Œ?{Ëزfu§?¬·-"Sæ'?¡
B˜
Ïã?ïù
²­ß?Bºp¹¹B?@²oΉ?:Ã;âV¬?7{^«ˆb?/´A5ãeb?ï¥thT³?€Qì¸þ?k;ÅGW5|?h­59ì—?§é>££æ?wq×iB?îKfßnKH?š½`Ym?Û?¢RZJ6JŽ?•á3µY֛?'îo}ÊØ?‰0?tj?ïlí1Nà?€¶*õ#9Š?zEh(®+?h*«Œî‹?‡¡ÿ¥¯U?{æi]ì	HAGN3FGL J0226.5-4442@p_
߆ã´ÀP̀SÀ9ÙLvѵÀ;¶³ÑSDK?Ý~-Áü‡@É.²E?ÿF]7ãq¿âYËRE¿t¿è¯ÐôéeN¿´y´22hn¿ÛþÍýñªIAGNbcu?ïî Xigg?_²Óªt Ñ?&¢Ü-rz?"¦ý4ob\?_êô%W6?_ÿ£ë?ïSc™^?ŒòZïÈvè?ilцè3}?}v"ÃEY?…ò·ÿ?ƒÆpŽqÁ
?îú.Ò¦U•?‡»oÝ»?Û#ZÛh?k¥þ¨ü0è?—Ìœ–È/¹?ƒúùc¸õ?îM 㶄r?›¢ 9ªr?XÒOây.?bt[i×?ªg_Eñâí?›'ayßÃ?ïø$í­²?KE[¡á£?ĸ£ºšì?á:xÙú?K•04¢:,?JYDzãí?ïØ@0ä¶?lfƒ»`'¯?TQ<Kš?Rþ¡kÕ¦?m€>/¹Ì­?eaÁÛàò?ï•ÃŠ&º?p9،ž1?s}cþ	4?V[þ5Öø´?
ÞÁh)?l&¶ô+Š?ï¥È–Ý&·?s,J®Ëj,?Yëïì{X?PŽ."°3?ƒküÉXêÎ?q'Ö"ª|AGN3FGL J0227.2+0201@d¢æàé´ÀJh˜Ÿž–YÀ9¦Ž.+ŒvÀ;¨è»?܏?ÐSkŒ–@	éôZ@VOàh
*¿äÂÖxênì¿ã¥ªbÙX¿Ì~ê­¥¿èîðL7AGNbll?ï
[²¥¦?)Ê5Ç?jÉ|#|²ß?ki‰@cýë?šûZ TUº?›¼éLV½?î¿Qí'?©?‡QÞé?³ž?«š?"/3Z†šu?¦;Àu{'?¡×R­dI?íýäÈÓ)D?—†QXÜ;à?•Ä:ݦR?"'€ìW?¥?–CŸ?'Ÿ*‡zú?ë"´'0ƒ?¨ÖWŸrM?ã§V\\?‰aAÝq¿ô?¿¦`…"?§Ûcß©ó?ï³³nµrò?"Nù+µCy?UÅË`BY?Y­Œ[먣?€Zjßޙ?'6}Oj9?ïi-Ѩw?‡Nçè³½o?xq±»QäÊ?rg­ñçϸ?‰{²ª–ÿÒ?ô@tpï?ïR²˝"?~!6Ñ	ë?z³b¶0?pü›Ú¯?‰ØÄãÛm`?thlú÷?îŽF ð?ŠO/Ƽ?‡òm¡7Ã?rW´dÙ?¡"@N}%@?†Œ.^þŒ9AGN3FGL J0228.0+2248@bɸ!ïÀAq[ßú¦ûÀ9´Á"tŸÀ;–[ßú¦û?ã›@§~ÎV@z¯Èe@öÿ /Å¿àÄø5û:¿Þ*ÀžýAñ¿àøº04s¿ìÌã6àVAGNbcu?ïÝð†Ãܗ?k<o•¹¹?jìöƒ?"%?hò¹¶'—X?LŠ
6c	'?EP:rE+~?ï(@\LÃ8?•ei…7‰p?vüêDTŠE?y%âû{?•8¹ì³Y?'tµMn»?ìõ±&Ëh@?¢>Ë5Ö£&?°³"¨\¼*?ž*'Áƒ?ž}PŠGqM?aÿXÎì?î£kaoS?" òq¨?}6D´1Å?tY×͵?¡Ù£ ¶@à?''fŒ¬S?ïæÔs<ì"?lJžÑ;B^?dµBÀb'á?kr7Çkà¶?AÙ(ÒTå?6KìF ‡y?ï±8‡0
Š?}zŠuec?f
I{Ö?aJIÇîši?|^¯Y:¬?wÀa[›üZ?íƙPû#? xçð°$ø?ª'†0¯˜?›öÐê.U«?'	Ó@îØq?‰+¸s,%+?ïša÷ì¶?s¬Yü›3?sCàmur?aªrY4¶Ø?³ïºwi?nxÓo½ÎAGN3FGL J0228.3-5545@qc²?î,™ÀL<—à[õÊÀ9!Å;ÞÓ`À;Ë®4[Q_¿õcl´3Mà@÷°(§>@h)@@6ý¿â}KÌ ñÁ¿æ'
ÏfÛ¿äŒR•	x5¿éö¥8^@AGNfsrq?ïùxOO§?K0dŸOá?&I[{$?&QŠ͚?DŒjÐÕr¸?Gïgˆ<ì?龎A'?'¹žR8÷?_àŽà'ÿ?c¿eÕ?6 Þ|ä‹?ª&?"î?ïŽRÏÁÛ?>A Š#?ƒ¡†ɬ?oø;°Žâ?"]§Û8»×?{`%Ï.fD?ïù}ÐÝ ?TŒca†¤>ÖÅÁ4Bƒ>ñŒÿ"©O"?KÌ}' Âc?T| LÙ§ó?ïüWiüр?Z*ˆçT?!,%÷5ñ?/§¨øOmì?4®›úÆÑ?VvŒª×?ïáÁ÷KÀ?lÌ8×ç?MÑJÅÞ¿C?P^BN=j?fɵÑí¢Í?eƒ\;û8Ý?ï™-¦+xT?s	÷Td£?tµ©~ÃÇA?fgc©ÚÕ?~³ƒ…³?l4]žLvó?ïÿ)aG ?*mÛ2h>£p9øÑ*>´C©d?¨ï:ÛÓ?*hÌm΢AGN3FGL J0228.5+6703@`†‰_$RÆ@Ë# C+úÀ9‡½Q.ƽÀ;6O¥YÁ?½Š|lã@
òê|‹ó@ó° ™¨ˆ¿Ü@YM	"I¿ìP|V¿à*rހ¿¿ïÿ€m•AGNbcu?鑠Ñ~?Á€s;ûŠ?™u"¶W?™Â~DZ?ƊÌ	¶ë˜?ÀµPcXÑ?áPó96ò?ÐËQ³¸?½	åË»´?´ÌâRbQ?Ö £U–?;ÿú̏e?æNcVLÎ÷?± Õ
'‡?¿Mc?¢ñZí©•?ÇFp¡As?®²}å4Ø?äM2…/Í?·F5‹o?³Ù§mƒh?¥]Cy¸?ÒÒûÀUE,?¶ŸÜ+áñ|?íˆÑD?·QNmÍ?‰ìx¨wÚ?ÁÔrÉÑ9?°{è¯ô}U?µþý§"? ?éЋ³§â³?Ç1U‹]þ?®\ç)ÍâT?­qúï\?Á&—gÿÝ_?ÁDL'E>?ëRµœ&J?¥,Œh>ð?³8(ä-o-?™f"ËfX??²2*:¢N…?œŒ  ŽŸM?êà÷%)Éí?£:õ'qdÐ?§Í‰%Ò#X?'ßð›,?½'D¤…í? ä5AvAGN3FGL J0228.7-3106@l«µŸôýmÀQ| À:Èá!§¼À<®ÎµY¿æ2¤[Ù3@d
‡ÃXZ@s`ù•¿ãóåVO ¿å'™³£c¥¿ÐZJÂN¢-¿Ý83<ZAGNbcu?ïK¯ZÃgk?½—ë{…ÿ«?'›«£¤Ó?½›õšK?s¹¤É×Q?'GR¹†*?ï‹ÑæØw?‡›Žh~?h€@ŒÌÿe?w:CWI'9?†ëv`M€c?ˆüéŽé+A?í¦—ð][â?šånçæÄö?™ ‰É~?'N-¿¾·Ú?­Iöi	v$?™ŒTR5ً?ï3q½Ã«¢?‹0˜Õø7?=&­¸³|?C[èúâ'?™-Vë?Šíj
¼šÆ?íè
M¤?ѯ—–ÎÒÐ?¶Ç¶n?Ѽ=u"ä(?f5Ä!?zÑ–P]?ïÝ>zö&Ÿ?pððÁçË?Q™ªëaq?TÆiZ{
?iô¯ÂãXl?iàÛկƖ?îךÁ{¥?'Ù75é?…Lü¬GY?}}ñ¶#ݒ?šwŽU8ƒº?M'49û?ïÛ¸vî7Å?b·f€‰õ"?,ÍlgÀhØ?!ŸV_Ó'?q=Yû¨ã?b9/1×úAGN3FGL J0229.3-3643@n~9ÀëíúÀP̖üõŠÀ9&D7guÀ;ËW`9%»?á¹ØRUÒ@½º@N@Oß_¡{:¿äpô(G³¿æ"þnIM–¿èÓŨôe¿ë¸V5õ8AGNfsrq?ïù^!2G?E,"Ê‹H°?8nN-ñJ¯?;> vÓJ?< ¤@·¹>?6h7«e&ï?NUè.?"¼ßÇ?bÖµà ^ó?eo½"Åݱ?ƒ¦~äGvç?=|‹ºq?îÿ¸ðTš?†é¤§rRá?Žöª›éb×?}S *À?¤s'HíZ?|9'-s^?ïèf¿Éü?oŠÎÌÌ5?#´_gRC?38÷Ÿë?f¦XÜr²?o.h…¾Þ?ïû(
=Ï!?9°¢7£?6Œ3"ÐÃ?1tB²ò?03–ñ]\W?'n0*s?ïàz{òÙ?k+ÄtÚ5?N×͑ìTK?P/:óÖ4µ?gϐä ËÜ?eü>RÅ?ïo¸"Üp"?xV°÷;XÄ?"Bz3,ê"?s31"ryt?žÁ*½ý×?g…Õ•n_?ïüÐF?C"6Ǚª¬?7dz"eÔ?SGr4î:?6ÖÏ*¥?BŒ['܍AGN3FGL J0230.6-5757@q…E€<ÑBÀKL®¿›‹âÀ:Ç1Ç"háÀ;í´£á8?à _ŒúÇ@¬²£UÚþ?úõ@|òÅ?ßîCÐuº¿äÝþùDп⏃0 ¯"¿æ5²%AGNbll?ïÐX§®Q¯?q3Ý~ÖÎ?8'…5\ˆr?5»@OX?vJ"·®]Æ?pùé,(Mä?ïo½ê²½?–ß¼Ó*k?m%H¥Ö'?r­6þ?ŒÇ>tX7<?"'ØN
~?îh÷·Õ?ŒÍÕüÅd®?þ9np'?zØY^D¡? ñr]-?†EÁ–'òï?í£GìË?§°ÂÔF*ì?sµÎXë
?"XŒE	;?±«àÜu͒?§+ì]!~?ïðÏ0²Øã?S	˜Üº"€?+";+?$€0§›?ZéMÒÁçj?Qö³-Çìò?ïÕ7—x?sàÏmxïÏ?U_²}û2X?XËÞSʏÖ?pGÓՇã?o¢þL.?ïVò9»/
?{ÇûÐ"`?€À&Xh?q¾3ÿLV?‰ƒRôþM?sd½`À*?ï"X?dÍh?(
´¾?b
ùtè?h,ZɞÑ?†g1½gT"?}ú—Zo AGN3FGL J0230.8+4032@aÓdÜY2À2€nÿ'÷À8ìÓXØjÀ;ž–"ì"?д>Ç¢'@z›Alo@e# ™5¿å©À‹Ôg©¿èqSlŽž"¿èé"¡¿ÝûžaTƒ»AGNfsrq?ïùFfQÿ¸?MCÂmÇ7M?#Á,¤©³?Š½"? @?F!5ÌÝXš?L£'ÿ^e:?ïw•<+™%?'€Š w;B?lZÉÕ?›?m6—©Bñ¥?ŠúZ:
`ô?Žý–¯‰Ží?îú&{ƒÉ?†PqNÐ1V?…ÛªžK¾?qf1¡.§?•Í[=…?''¾äÐ?ïÍäÎö?u5î'-?-·œ
?3œ	þ¼˜?x%ë)·¼ù?tÚÑ7䟇?ïý]˄š¦?4¥ÒïãV?é¸yé¢â?tNɺ?/®oªÅç?3¨Š»?ïÕ-8P?rŠß¸?Wcv²çÛà?W¢Rå€?oC1Âì3?këÐï)l®?ï•.Aºh?kÏÑv{š?uÏ&†p'?ZÔä¿£ìž?¢Bµ/?ê?dÆ …=Žx?ïø—Q‡ƒ?S94ê™l??ÿå94?,Lp{)j?K_Slú'O?RØëÑæ5UAGN3FGL J0232.8+2016@cýŸÓo~ÀBNº@NÀ:"7ÜæÀ;¦7¾³.–?áæ'²ƒ@)@Í$¶n@4ßxöâ¿Áô©Ú\ ¿èßiKaí¿æ¤ç¢Þ^¿¥g7"
`AGNbll?ïçô,Úuú?b]Åè!?FÀ`I6c
?HWw˜X˜=?b[ºð½&?_N¤2æ»?ïd‰B%?'íaɜâ<?k§öxr¥Š?qDÀªÑ¹"?ó±×¸æ?5ÁHu?Mó?j©Ç-3f?Àñ$ÚzÁ?€oãm4x?š§Œ\«bÖ?ˆMÓU€z?íígóVé?¢úíÊÝÚ?pá‰Å(?z¥X¡?¯
]âc€ç?¢—p¾fÕ
?ïÝüxzÕ?«d+…Œ=Þ?51p'Mu‹?6cï•Ô%D?p+jÊø®÷?«f.
sœ?ïÑêƇä:?o:å|©?Töˆ×°M·?Q?VLÕÖ?qÌúÀ·G?jN×Ö™¿?ïX"à÷ì?'`Ýì~ö°?ƒh‡
µQ?sÏ%<ށM?†vljKU¯?|ˆa©¹Z~?ï™.5)q?€#e³¬ ø?Zҋy'G?]|Ã;¨Éu?†Z'´g	Ö?~¢ ÚÓAGN3FGL J0232.9+2606@b·žÀµgUÀ?n¢ ©XSÀ:Š°¬Ö)À;ÔîµTá?ݑwÿ‡o@.Ò¶p¿Ü@°ßŸã4ÿãë`FøÉ¿×Zp,>¿Ýc²£<ì¿ä§¿ zšŒAGNbcu?ïÃÖâ-?zT𜆛'?R_U
Ã
?T&'ðÃÜ?yå§ÁOî?w×öë?îNå3~1?©цùa‰?ŒœÌ,}‡K?ŒÁ͎jpÊ?£êyºcæ?¥–ÄT5ë?î;InÖCæ?"#2è??Òô÷;Ê×?z}aWgú?£áîšmx*?nT­6?ì3YO7ÜÌ?¢?ò}CIA? íå0§ÚÓ?–
´QÛß?µîBî[³?œ
À[!?ïêË^¸?pž‹Ï·!è?7¡Ÿ%¬½?CQÍðp˜?bùë¤Í?m"9òåÇ7?ïz"la†?É̸?tã©©x\"?u"¹yš?‡ÆMʆ?ˆ"ç_‹Ø?ïU8[' N?y±Ò¢.%ž??Iþ(?f>MjÜ_Ä?‹DBBÜ?v‰ìé¨?VX?†XÐ	%?•*G TS&?|	Åzh?•DÍ¢PE"?|ÌàÑæ	AGN3FGL J0236.7-6136@q³SX"ÀI¦Ò?ÓT¦À8…´~êÂÀ;"Æü©3k?ç}¹ÝÂúw@äÇÉ@w:ßyø"¿àp°F%ˎ¿æ£ªGDk¿áހM¢A¿èˆ4X'AGNfsrq?ïüýuGf?,.`S{?(k*Y¾?¤¶lòV?0Ê;SHÿ?&£çŠ&¿V?ï¤Љ‰›?‹Š–</Ç?c4÷E«·¨?}ýèwª?'ÎJQY?'«ûÍ¿‡?ïzF˜ß?"NÉ_ܓÒ?"âG†œÿº?r"(Ô7¸?"¿"i®ä<?€P¶0y?ïü"²àù'?Gø‰|¤|>ÑfÊsÖu>äÖIÌlÆ?;ѳð"ž?Gç¦á§Òì?ïþD[¤–x? :\?oSÇ?
ÏÞögŽr?!8Ãóî':?á§^NC@?ïá¯=Öá_?g$WYâ?Nk‹á=?Nn܇¡È?fµÿˆ»?Ò?akú›X]Õ?ï™T;9½?p교z
?ugª÷Œ?c³7e`?~;IºÛžý?gAÝEú?ïÿmúÀŒ3?#©däu-±>Éí89³>ç–AVa?qEs׎?#~ÐÙzâ8AGN3FGL J0237.5-3603@n%ËßÒcÀPr¨æj-À9êøš°ðÎÀ;ªÞüz9'ÀëhnSp@®xù¼?ý»Ð@Ô¿Ôûè]ê¿ÚkNûï,ҿґ*2w¿âÞM[ä"yAGNbll?ïÀL
Ÿ¥Í?9{›/²?B&ôˆ|œ?@n¢ٙc?}–"6šO.?}½Ž~NÍ?ï"ÿȑm•?Žå‰Ÿ5à?gJ'UË·?ùôˆµ"?…»&Ñì?ƒï5ÆÉ?î'û<÷­ ?y®6…?=l>ù'?|_3SÀ?ž!Ч{C=?ˆÉ§¢r?ïk!é½Q?"X½!Y?r«(?½+´?'"B`°k"?'þ­Î›w?ïßÙQj€Ò?{}È÷åÞ ?6姝'f£?=;Þ%Å]?mIùÚI]?yܘû™¨Û?ïßd²½U?lpÿK?Põèò>í?QÓkËøµã?h Y%Ýø€?eA'
݈ð?ïi‡I8&?zC‡]9¾~?Pçe2Á?i…vøá?†QÝõ?tow¥´(?ïß-%ì½r?j©¯VéGŒ>С
ÉB'‡>ÖÑÙ63ò´?peDÓC´`?j¨ãÁ3#AGN3FGL J0237.9+2848@b¯8¾øγÀ<…'ßBñÀ6ë7OËÀ:ûìƒKy@6?çÍ@ h(,ºž@*%³Bâÿ¿áêÀӚF¿æžºæÎß)¿æŒ*Š¿ê½ucÚEAGNFSRQ?ïÃpaß:…?v3)³wT?q빪Ž¼ú?p̈}K ?h¸*ÈèQ?iÖÄØÄ +?89q*?ŠA?.vÝm?hµá{Ð?|tKÄ$;?"d+µ"Ԝ?€v‡cf¢»?ì¡ï9;én?©L½¯Hª?°ŠeØ5±t?£\m,ZÕ?¤Ì@½Ô9?šÉû= èp?ïö"\×®?a["¡¦¿ƒ?SET±|?KØG¾IŽL?RÃìä?_oéØs¢?ïÜ©¢z?teïq]'ˆ?a¿EL¨¶«?iv?J¾?a—·)"ÿL?j+¥ÓÂ=?ïۗŸˆ4Ü?lJG±£[N?S?ýwã²?RRº
2½Ÿ?jÈaâTê¯?e>ڎv¼?íBnð"½D?¦Ý­8Àe?®£8¨ãÅ?¡'†¡a'?šk°¯6r?–¥\ª×®?ïýµ|Æq‹?Dh%Ú5eE?pÀì-D«? ß»Ìaæ?.ŒlVѧ?C@«ôôAGN3FGL J0238.3-3904@nþã€ßÀP0‹À'¢ÜÀ:uå"m/®À;÷©4AP,?×Í/@Ð溉©7?ÿ] D-¬?ï÷½À"-æ¿âÕ -qþ¿Ë\6;ÙÓ¿ç8€šR¸AGNbll?ïÚý	*¡?sšY<?2ßùØã³ä?4:Dg5Øó?qS{ÆSšµ?rÎJg¸?ïR‡žM?—+þ÷Çk?{ˆ®´Žµ‹?qßGn?–³'ó»ñ?"A3½_?îÓÀ•B-?ˆê¦Lf};?Œ'`ûŠ?ztŒ^
¢Ž?—Vd½N<"?'t¾Áü?ìêȱ³?ªÃèuq]?ˆ¡ƒ;ìç¶?"+G"Y¸?µ—ÑWˆîu?©M󼁤?ïò]ž§Ü?Ydš?Ñ)?#Öî ®Å?$b¡ÌR
7?XÉåJ÷¼ç?XãwQ!Þ?ﰂ¹O¹É?|µ¢iB?fߢô«ré?cG(ÉÒæO?|NÑоÞ?uΤS·@?ïrüF'Ò?yCÀ›Ou?|Qðtßx?e²¿ðB`3?…ö6•¢Æ?u)_ÔÊì?ï:&©¦Ç?‡Ãôíðaf?{ÑãO'þ?j‰Umá€?'Ê¢kž`]?"¼R?˜AGN3FGL J0238.4-3117@l¯¬ºËCÀP•‹B¹À9XõL»šÀ;hœøɪÙ?Íè»q@ñ@áü]‰ ?ý^%y¿ÒúÁ?ƒ2¿ã
ù;H^¿Ðá¢Y(1Å¿ÖwÑýÅ­AGNbll?ïï–( ­?Yä±,ù¬V?=W9à7ê?9šJ-¡?Y}á"û4?VáўE3g?ïyF§Ñ?ŽÊ4'ä
Ú?nWà'U?{òIP}?Šr¹¤è?†a
nм?î`¹†Òu?TwUÀà?'ƒªŠÀ~?€Yw8fÓ?šÐÍ+z(Ñ?‡jõÃñCë?ë¹yœ+ÍÂ?ªÀfPÛ©x?h¤6$- ?i¹ä+ÿÞU?À·ˆµú+?ª Ðhº]ò?ï÷7w™O?H]˜-?5‰›Ã?2i›g
?H]aU¸Âð?BˆúÎ—Å?ïÔmÔނñ?rü¹Hx?V–`eV­?V/¹ay,h?p#}sIT?l»ÖM³ Ú?ïd䦵P?y|Ï01?'/ŠæZ2î?qG¢ÇcØø?"—p«€û'?q–(È?ö^Ê?‹ËØ­—®?d=h&>2?Uƒqr1Ãk?¢àšUÜÝ?‹V¾J€EAGN3FGL J0238.6+1636@c˜à¿]xÀCÏߦÄ%À74^¬]ÁÀ:¥žÜÏyO?÷³ÿEÅÝ@!M^|Y@…Öí¿Ý諍ën+¿ãÇoܘ&¿â6"׿æªÒîò3AGNBLL?ïìË%5w9?"H…6¬€¤?-–¢v¥ÿ?ḰD%ö¯?a[pbï["?'—<'ê?ïŸvɜ&ù?"äçýãm?bø5gµ+?dÎ)ÎÅ?ƒ›kÈ{?'`耻?îBä"è՗?™ç®¶q§?Ž¹æG'i?…s€D!ܸ?¤#=3÷…0?–R"fŽ?ïý8|ô?L~EÓQÅ5>Á˜h§¡Ž>í#a9‹?7kÏ_@»?Ls+tø2?ïû0:/{Ä?=3Ö^?#C{FÛ2ß?íU€÷?<Üp0±-?:'Ã<Àh?ïÞÈ˓ð@?júá0$Áœ?P'›ãüõá?P¬¯¾é#?i#f@4¦5?d):\'lî?ï½Hí§?'yMgʑ?…ö̙ƒñ¨?'gKíU
?"ŒðŽ©îª?BqbÅ?ïÿƒ2Ïàþ?"œ…ÌN>¶rD^ª>ÖÁ«øÿ¿q?'¿ú¾¹5?!òsæAŒAGN3FGL J0240.5+6113@`õ¹pޏ?ñada(ŽêÀ5xþ'jöïÀ:%ÂÐʈO@K4[Ò9@]Ë5ó×Ô@N
Óî$¿Þ'Q¦»Á¿åt÷ù¡A.¿æÉÀµg¿ëS?bk…	OTHERHMB?æ±®ä¨Ð?ÉÔýa®àm?ÁÃïñ'Ó?ÆÓ¼¨ðØ"?ÃuUÏaÉì?Á¢›ìJ'?È1àbUà‡?ÐÿÔƒVj?Ù;†á'š?ÐéÚ}ÿ#%?Ú«ˆí­u¢?Ïh÷Ž«?ܜ"·Sœ?¹¶žÄôÇ?ؤyá1M?»Y#÷oÒe?ƇŽÐÎö.?±ÁŸß¦:´?Ëèñ]GPC?ÁYBç[Cs?à›¸oó'ï?Ìñ‹%Á
Z?ÐÔquR?Æ¡\{Öæ?ìâô¯o›?»Ny¤u…?¥ECS'W4?´îp³Ø*?¬‹q°îá$?²²þäYØÐ?Â^[øEÃÑ?Ê~óçT?â}8él–?Ͳ²!¶o?ÑÖ`ä
Dì?ÅÃjxnÒ?ßþWOXi	?·{0˜'@?ÖC[{ô¨?·¡ýsyBŽ?Ã|šigŸ?®Lql°«¥?ÓN§UÍo"?»œ•ʵ×?á3l‹eñ™?ÃÑ\ô¢©¹?Ĕÿ&ÍZx?¸
¸z6P?MIXED3FGL J0241.3+6542@`½œÁæ°@Ñu @&âÀ9>$'ýÀ;9ݾŒ˜)¿ð Õugá@{«Ý>@£Gßg¯¿â:ê«@FR¿ãu.å4'q¿á}.\'[¿Ôb³ðC/¼AGNbcu?ëÞøӈJ3?¸×\'Ž>?BÅÏcõ-?yÆêXЅý?¿
Պ"?¸zèÚoŽ?넗Š±Ûk?ÅbwY†b?•:4…øåË? ížq£9?¾Œ¶‡;7?ÂÝ yišÆ?꽆¥Ãjñ?©¨‰"œbT?¦Ðû°?'N"Úå`º?¿Dè'P$?¥Þ5üwp‹?ë:ã¯xD?°¹†B%ž³?hŠ6a}S×?kƒ'Ç£r?²HiG¹Ÿ?°¸]`¨Ñ?îÒ4[/V? ˜!Ö[Å7?sڂçTN=?t'I߶Î"? aióÖÕN?Ÿ/J*é?îë°w²"?§ëܦH?y°Óåe?'ßÈ&p¿G?œFR?€ ?¤ ^Z®k?îJ%­(?—=c&¯°÷?–¼âCãvá?†f'HVß?¤<î_þõ?þdü,V?aÒ5 ?ùEšC¾?Hö\8–fÛ?>áˆ&'ü–?¦àooc5?ãg3ŽúdAGN3FGL J0242.3+1059@d:¬ÿ§ëlÀE¬×5ÜÀ9£YË8À;–¥€éŸ?ñäŸANSö@Xéçå¬î@N_ƒô¿ãÔ—m[¿å³{œGb¯¿è¶8¤ißË¿ïÿò"5£ÀAGNfsrq?î Ø	8Z\?®W9Tày?¦
ù"ñ?›xÕ6Ýö?¥ŸxçÙ~È?©Þ0;Jóˆ?ëiw‰4­Ã?µ!ÐÔ&.ÿ?ª•àÖ³Å.?¤ÒäGu‡?·iSJ'»Ó?­Ð±ä¸'¯?ì–…	Œ?¨""¨]?²Tý®"/? /F%¿‡^?«Ëí³/?ç,±KØ?æŠ%c´'?¯ÈÙaÖjÎ?ÄÜY¹è'?© •@q?ÀûbV·FÔ?¨6ཟ§3?î÷6¸x×Ø?§¨æÓ.ä?ŽR$MYÕ?Š"PRª|?™5"hUŸ‡?¥'þà9I?îUµÐB3?Ÿ"òÒ[?šÚá]^?'µZÅga?¡}72M-{?"ö_"Ÿâ?íc@Kl†?¢øg¹/ñ?§m™dÚ9?™W=pÒ9Ä?¢^aåAE—?™4'm€U?ì&öü÷?˜Ï÷PcW¯?µ,uic›Ü?'Ò×Tšsû?£7¥a7£;?Ž`H«o£àAGN3FGL J0242.7-0001@e"-@ªêûÀI÷˟¦#À9°}IúÒÀ;ɑ
ÙÝW¿å˜?	ˆÈo@
ΛzšOø@–€"û¿åsŸi½2ü¿äf>"z~¿åÿC!gÙ®¿×0T[¡çFOTHERsbg?ïg
è*:*?¦höd_?~a½bk?—n¾±?‡w­tD?–àkìp?ïžyÁ{Ð?•ø{¨øG?hŸb]ј?ƒp˜ÉìÇ?'WÈíÝÒ"?‹N@¥˜Ÿ?í¢­PŸo?™'|$úÇm?ž§"}x‡Ã?ŒxÚW
/?¦ƒ2ë]Þ7?¨³Þd ?î€þ¿Ûo?œ¤fÁµT?`Ø[YÙá?b¦_<™?¦âŽN8§y?œSÃï=?ï'-ÙpãÝ?¶';
ö†¸?|ý̓}ŽÑ?¯~[ËcÞO?zkEԎ¢Ç?¨-û=‡ü·?ïäçàh§?iÙ7:ë§?JýïùJ£?L8Ѻh¸M?dXßCñ÷?e~©ù˜?ï/×=`€?¶3Rdzí?‰Lø¹@§?zÏ	š?Š¾²–V?qrg
›Ã?ï¹mÞ;n?sIð"2ÿ?<\…ñK|?2Ÿ)9€ód?€Á¤@ŒÆ ?ré¼=Ó¶#AGN3FGL J0243.5+7119@`wL Õbž@$Ê· "À9h±Ä2ÊXÀ;r¨W¢~E?ڇKBƒ¶@}™èÉØ|@ãV€bc¿ÑÍ8[ÕØ~¿ä6Re¿âtÛ6ûrZ¿ã£üH‡Ð'AGNbll?ï˦Û\÷?sú‹âÏÖ?bÅ@ºMû?]÷5Œÿù?q)/œ£UÚ?olã³çB?í÷"ŸQ?µZD'™Û?¹žœ¸²ä?˜3¼ÅîŒ:?¨˜^_u /?±"0i5jô?î"Õàß?"{*ù­õ?'\D_¼N?ƒB§<=ø?žÿ"0ŠH?YÀÀÃâÀ?ìþ
­EP ?ªÔX¿9?zËät¨+?‰Î‰´ý?´ 9ý?œ`íÌ8â¦?ïãú-ƒý?•¹Ÿ‹…‹™?[öÞº™?ŠdEî¯r4?\ú®"uëÜ?t/F#ƒÈ?ïj½sÆÿ·?•Ø²~Úàé?všÝ"Ú¾?yVŠOH˜m?ŠBU–Þžô?'eñqRñ?ïk•éûu›?'*Üîé¼?€:ü§o=û?w|
7kC?"߈Ô3û-?yp;ðzµ¬?ï&'HÕm?€­ý¸'ÓF?ΨCÔ^È?a¡gÍ#sÊ?"Hpÿhø´?³
CraAGN3FGL J0244.4-8224@r©óà7ÝÀ@ßL߬£bÀ:tÇR9‰À;Ă´zÆp¿ø•€Túe@¤ççÛF@n­ŸàÛx¿ëÚåÇÎü¿áwëøÕþ¿ä8_öhZ:¿ïýÀÈÐÇAGNbcu?ï"Ú´°»
?ˆ8Ê<rδ?‡múK¹{‡?‡
&*©OY?\ÚÄQ<)o?`Rµñ_T?ïÆñCk?œ×qdî¦?x¥ïqŸ ?‡÷ïÜ?–}¦z§?•—\PÙyh?ì#ÑÎ5Ïè?¢n))?²o™á€?˜oÞL`‡¨?©ºí+"A?–§ùíô?î­T!{Œ?™ö(dïš?q/ñ7wÔæ?wPm$¡m?£외ü ?—­ÿSÉ?ïÁN_?€÷(îô-|?z;['ôN9?€¿chì9?Uc<ŸÊ^?SlÁAÑÎ?ï¾Ì2aëÇ?~´VÉçEn?`Z¸°0×?`ø;Ö9ñà?xlŠÒ,?y*QýÖ2?îž[`m?–Ĩ™Š·?¥Cßå̘?"nfÖqé?•dtЊ½ ?ƒÂVÝQ?ïºÃ`	?skFY‡"?;¤‡ï؇?L¬Ð|S¶¢?€›{¸Ÿz?rưہÿËAGN3FGL J0244.8-5818@qf{à~íÀJ‰~¿ù³À:Õ¥¹cÀ;©ë-àãÛ?ғ&
ö4@
˞¤pb?û-í"Ti¿ç«/lìâ¿âˆÓƑv¿ÝE'"&?¬ùËÏ÷¥AGNbll?ïퟕ("?báú©zrm?,€V2È?-0uqNÕY?`˜jÈàSô?aÿEšOâ?ï˜ý²,?Š»¾3a>O?goÞwÌ?}»ÝÝ/Œ[?"1d»9Q-?€d…YQp,?ïۜ?ß?"‡ŠÖæ´³?'ìÆ5ݞ3?oEbÏq܀?"ÇAv³?€J"Rƒ?ï@ҕ[î?•dVŸ??QÆ¿¸L?P™CÓRn«?—hf9Ӈè?ŽÃéËÌvÛ?ïû[fÒ¿?<` Ti?yÒóba?y둣Ø??Eæj'?9ƒ€˜r_ý?ïÞoÚáëö?jì2ÖsÞ?PqwSÇ?P֎þœ8ì?iWš½N^A?d±"ÇÛ¾Þ?ïšÎ€‰°Ì?o†'Ê«1?sœ":Rõ?_{–7³P?~ü+rg+(?gUꀄzD?ïÛ0k"Ýÿ?e­	ù'?.ÁJSÌÑ[?2"·P¿¦c?qq¿ÂA"Q?eœbœ6hAGN3FGL J0245.4+2410@c7oŸËÀ?ȑ_8t¼À9)›«Â'
À;'ÇÖÃƔ?ðL"èÝy˜@JÃú@Mx@¦v pMp¿ä‡mÉqȿ稦&𯫿ꮇʅ¿ãä¼òAGNfsrq?ïùSû©^?@ݲZßí?:këüC–?5E5ÍÌÃÇ?;Y¹tÕ®?6v‡ÜXâ?ïW§°ó'?'\~»YÎL?q 8ÇØ(n?pPX8J|*?¢ûÒz´ó?ŽÑT6‡'[?îšÄsÚ9¿?ŽËjòÉ(?"D{!aä?ƒ<NL*±H?™böh~M÷?…xÏ­Nm¦?îÎï3K~?žäËNÐü?‰käÓÊZ?"Æ¥LrwÖ?¨®ör<ƒ?M·÷Dô?ïü‰PÔ·Z?1ÒIë.ØH?(àEË$)ª?$%ÁS–?.Š¯ÝÜ÷3?(>ÑXøÉn?ïÄÅ1Öok?zÖ<Éõ+
?\`æ…ì¤À?U{:"Žº†?v…-Šªxò?wžæ;öŸ?ïZÊ@Lî"?~Ù~øŠÁ?ƒô«¿àþ?vM>óíåW?…XÄ.œ	[?ré[L"?ï‰Ø€'?i#dq	Q?t"ï'ø?eÿtn®µ¾?ƒ^ëê?|hÖ·iÁAGN3FGL J0245.9-4651@p]_Œ¨ÀN
dàTiÀ7š¹y2ñÅÀ;F{jÚin?øeZ‡àß~@imãÞ6W@ÊA€h¿âißW=ÿj¿åðxô'˜¿è? Ÿ»OU¿éåb¶6;AGNfsrq?ïéaŏ89?cš$ØtDN?\KrÀ¡ü+?_¬ySÐx?Pñp¤?MOðbJ«ç?ï"Ï›Y–?‡°w†¶?fMÍT?ji®[ÓÔ?…x¥ù¼SŠ?ƒN8ܝ?î°@Ó7}£?•OK¥ª?—·´F?Ž'® ?'ö."Ó?‰¯@\×ëf?蘭@;s7?‹&Õñ}u?R"ÃD°'˜?^dfÿŒìN?"…—‰=
Ï?ŠK¶*ז–?ïôžÔ},?Q:§©!U÷?OZ²—í°£?L°žÎ½!S?@VÒS#}©?74èÁßš?ïÜ^*?l3¬ty?S%Û.v?SkÑ¢û?jög£ÆÐ?d"4Z`*Û?ïž×­6Á?o
¹Wù1?'@`'fús?‰·¬‹+J?‰Wˆë"þ?ñy>Ú*3?ïîZ'¤‹C?iÿ-賘?;LdÒ`Ú??®zŠj?\w¸ïXf–?g§žªN—nAGN3FGL J0248.5+4232@bÏÃøÀ.—VgÀ9û07EçÀ;Ö4O'åJ?ê¿7öûï@
'­õF=§@T̀K¿Ç¿éê7§ó5¿ØtKR¿êT™"·v5¿ïÿتrýPSRpsr?æ癝±'p?Ȇ}8¡x?Ê
•ìL*6?Å+>½U
ž?´®:I"?¸'Uɋ?ÌÆSêkvÏ?ė/eP?àþÀŒˆÓ?ŀå‡r"a?Ï>©çx'b?Áh¦ÿÖ?çpOFy?°"Á·ß™?Äd\*Î4×?©`e—õ¯¹?¿3Å2b‰?¥Ÿ?´6X?Ö¬öf+áŽ?¸¿vŒŸ?áø¿™Tò˜?½4þ÷†?µ†)šñ?¦Êò²Où?êP8'Å?Ä3MÑwµ?½±$îªu½?½¸ÅÙ¾x?¯š-Âw÷?¹ŒvÒa§?á³gj6Cx?Ƶ¸´$?Òý¦x>?Á8%¡E'?Ã7fªÀ?¸Bˆaâò?ëh•(?¦QU°|-O?¹µ¼ =sd?¡'Ž‹Ú¥d?¬á?[ƶ?–½''t%?çZ8< ["?­;ƒ-¯V=?ÍÐ~#,¼?¬bNÌé=¡?£ƒ±GW¥?'¤ÏŸéS'MIXED3FGL J0248.5+6022@a¶â—?ç*‹_Ö:›À7рuÜ%/À:rgᐩ0?ÿXŽ¤ž@ÊÈ.›@Î`=Wyd¿ãââ%­W¿ä"Vÿ¸¿êµDøØnl¿ïÿšFçPSRPSR?°LŠ0}ÈÄ?²Ž>¤A?äÛIÔת™?Ìn~z¦²?Ò6IÊñ¢¼?ɝª³¥çä?l¯©¶?ƒõ÷‡Æ;n?ã÷ÓFõ™?Ã2ßVÎT?Ù§Öûœ:€?Ã4'¦,ÇV?ěiæ¬$"?­ìÿ>±c?àJT¯Q3F?µ´ï»³?Õ¡®‡*?³:	Ïj>–? ø¼¬Ì?bü©¨=H?ç¶f¼ÖN?´çmÎ?Ìè6`÷U?²	tcxL!?·ê9Eü "?»%Öÿ*Ã?æÅîÌqÍ?̄l'?Èó(+BN?Æ<2&ò?€á-"c?Ž^®·
ô?åK®­¹G?ºRÇ7·|Y?Ôá™xªX?º֍jâ!?Й¼c›?²Ÿ\"^)?àR*Å&?´rIóü×ü?ÎÌ
˜góã?°‡Û¼zÊ?­ûÅ:?"Ö®.o¢?çÂNZ<GÀ?­ÉFïùX¹?ɯ‡Ó¯¦2?©<}OZ2PSR3FGL J0249.1+8438@_qåÿ£¹®@6my€žQÀ:
ˆÊ>}À;鯣ÇÀ$"Œ"xs@Ҕ%'_@,u?È¿ßù7r÷³¿èÞ X7¿Ñô²_õDK¿ã&rèÕÁéAGNbcu?ïøƽ`•Ž?NAï¥R'?0e¢™-=g?4dy+¸»á?D²9\j?K…¹U£›K?ï±ILéÃ?…âêÎó÷?k™B,Z†ö?ná4Lˆ¥É?yŽ¸ï½$?ƒ†]Ö9?ï%iþ:Fè?"Mu&dB?ŠZj¼WÑ?qù)X0F.?'"h»$?€šÅ‰þ™=?ïâלoÈ÷?jYT¶4âº>ëf&ÞõÃx>ÿÖüÔ§?mý\i9ä?jKfc8?ïüÞVq?3ÝR8L¾ë?#ž³Ñã?*ºV(±Ê?.€©Å‡¼?):ÙÃ{­7?ïâ7È÷³´?p»-€%[-?Vm´O#?UÛ°·°Â?b'\ÝÉBØ?jª ´·H~?ï›ç!ë?Ý?rÌ[É6®?t*LË-çú?h£@°v	Z?}â"U/©[?h"Ëw­Î"?ïû¾¯J'c??!C"N>¸ÙG¨,>½ÅÝdP:š?@øû£ñ??
fï'SÖAGN3FGL J0250.6+1713@cí€í )ÀB‡dàTiÀ9î&'d@òÀ;Ÿ_ý–™?뿸Àâo@v`Y‡?ÿ½±žÉj¿ê77ÙO¿èM^»Ðù¿Â2MD¬Wa¿ÖÞº_3AAGNfsrq?ïçÛP?ªÝ?dšg¯B¡†?GK8´`~?G/_Gم?bQá¸,í?aý䢤€¹?ïN°ia9ù?"'mË8Û?rL9i+0f?€Fô^ Å?'–ä|yŸ¿?,Þ CŠ?î}ÃS–õ?•>ó6¥?"ܾKC?ˆM¡i3Û?œj×AùRD?‰ïîf¯ÊN?íĭݯ"N?¤ …X/q&?suÅ{‹ç?'ABcQ†ú?°£4¼¹óñ?£3Ök8¡?ïZʰ'?\|¡E÷?C(ºŒÂìZ?>bŠ¾ë?Vò-g•Þ?X&HRû¨?ïÇd±å&?x‹¡ÿÝ?\Ĥ(K (?Yº±S)ä?u΀Í?t<ˆ§>(?ïW¶;Շö?'ûÈ´ùj9?ƒä»%-?z2Ç5×B?†.VL	eQ?v"ÌÌë	]?ï`WR˜?""@ ir"?uéöUÀ§?r‹ç	{??Œõ>"?ØB?v9¤…À¨AGN3FGL J0250.6+5630@a[¦?šIÃÀþ¬@:WÀÀ9ŒEÅ.îÀ;FÙõª;¨À{èP¶Ñ¹@z<Cþ¬?ÿØրÂ-¿Þ\†öÅ¿èVF3HµY¿Í›Ý '¡¿ÝEX"ƒÅAGNbcu?ïjcØäÕz?‰5Ë
æå«?VcL*Mû?S±ö9,7?'Q¯û?ˆ8†d¹?äd.Öઃ?Øêª`﷑?›pDã>;@?¥N oHM§?Հž&D&?×Ý*í-YC?íVoý?œ$­á¶w?–-öYúL?j–Ä΋Ê?¯‡ޖ´ô?˜4üSPž¤?ïY9BÒô•?ÓhÁa>>ð
¬–"Ÿˆ?'—5>Ýû?"ÔÔ<´Š?ÒDñÆn?ïÃ4WËmý?x
	hfuE?O	>À&uc?Ià#FL.É?z"¬WKhL?vgh«x[â?èý¤eÐid?ÔÒîÜjh?–À6üt
?¢Á¸&偀?É1kÁÞËí?Ó¥i??ï+u¾aê?Š™ù"Ézs?"(,}b/Ž?rdÀ'-£ø?"{k?…ªÁ¥ dÄ?ïÙB¹/ƒs?gÛnæÂ>ËîÒ"æ<ñ>Ϥør{Ç?s[%x´'?gÚ¡50,AGN3FGL J0251.1+2603@c=X@žUÁÀ=ƒ?ÀàÀ9´üÄâÀ;£XãÆäU?ó³	ªx¹û@Ä;dÚö@J3q¿Ôö¥»][¿ÞAç«ö=‰¿ç{"SÈeE¿ïÿƒ€¨†òPSRpsr?»"9Í?®0àµÃ?èTM;¿k2?ÈÖ¸'Š	6?·æm­Ž‹L?»Ï˜¯
õ?ªóü	Òñè?µi|ùk_v?ç~Âüûyð?ÇUzþo?ËGõ
OG?Ã2ÏÇ9K6?Óôr—ï–?±'ZáîŠ?Þ®Î7c¢?´œ"?ʹ~d<ž?¯ÙQóG?½‰™ãø?§Ï'æý›?薧ö˜g?µ¨Ôuè®b?½Á/­7ô?ª"+y'­?ÍßÇ#H7/?ÈñA"—?å'ÁC۝?Ìpžª
ç ?¸*g£üi¶?¹Èbý·b?Áùbà}ŒP?»ƃ1£;?å.?>Àk?ÅtsUžSN?È	ä"‡r?º™§Râ?â,q*Ã+?²›"©ÏÑø?ÓÃ¥[Ä¡Û?¯ƒ¨t0‡?ÀƒË¯Ÿ?¤hÙ¦W ®?ÔåÞðՄp?¬ÄÉCF?â³ Éc¶´?°Éšæÿ0«?¶Ë}?žÍQNs¢ÜMIXED3FGL J0251.5-5959@qu€?öÀI¤¨à^z	À:phŠ'¿À<FJg,_?Í퉊¼
@еd¦GÓ@QÇߨ½¿É2Å&\­w¿äÍÎZýÆ¿áåǥϦ¿ïÿ¤D1LAGNfsrq?ï¯5ãå?še…1?yÍæøpQ?|Úº$c?m/ä."?hb*E¼‹V?íg¸.áC?¬"@­ýÑ?˜ðkÁm?–´%k\_ö?­"åWˆ'?§'ý{É؄?ë#δ-™–?§:ŒB?º›æ®}à?¢ ÕÔ܆k?©—Üí5µà?•Ÿ¸3æöê?ìMžÝs?¨š7_xó?£j`Zh?•Ãd—yñÃ?³Ýûh–—\?¢÷-.È{–?ïÞ9×ŬÑ?k·ìÈm%?có«Úñt?fÓÄ8ío?[¦M\)K©?RÕԃàÉ?ïAÿ|ªþú?ŽaÀöf	…?æŒZ!¤·?w"†Šì(B?ŒÚ› ë#?†ÝOè$àî?í2¥>ñàá?Ÿ¤y•™å?°çVú*?›¨f$S?–
ÿć3/?†~môCA?ï!;"ß(M?ƒöÅ6²ñé?ˆz¾lt¸Þ?roª²¥J?6\XQ—ü?9
+]ÁôAGN3FGL J0252.3+3830@boaŸÂ¨‡À2ˆw"^À:[àíìEÀ;Ò¡áf·Å¿ðvĖrs@'¶YÃÀµ@ø-Ÿ nË¿ä'†#+d¿ë¦Æƒ»š¿æ¡«;W™ð¿Ð–Æ\˜AGNfsrq?ïíۂzÍ?a'ªÌh?,?36ð'r;è?2˜JËÙâÂ?`†F‡w"ä?`£œ® 1¦?ïu_çÌá?ù[èY!?oÅ	±	6?v;zÇ÷Ææ?Š¶ÙXfíw?‰ã."/Tÿ?î2¹<eû¡?'ÀD||jn?ùµ]üQÎ?{óÿê"†?¤W'ŒYë?I#½ýڔ?ïŸdG/òê?~¸¡ºóï?«Á½å/?"Ò`}AZ?‡é˜*EÞ8?~¡©ÃëJ9?ïøPÃ*ÑT?Y¾~\§¢Ó?"–)˛?:BwC£³?Jh¢æÕN?S¤—iµ›™?ïÓ:Üc²q?q'[e`¿Ï?VІX/Õ"?Sú…§Õ2«?p®p]¢w?kùƒÆgè¥?ïX–Auk<?{!?x5{?~";ünqÁ?h2¥y¸±ï?ŠÑ›~ü(?uÎÑäؔÿ?ïðú''¯ß?R¨ó_´?µÙd)=>ûb¶'?]‹Jëómõ?Rˆ`"UAGN3FGL J0252.8-2218@j7ÿyÈCÀOŸÿå(
À7–>Õþ¤¶À;"™.9Ï?ø¨y @Ò'{™ÿE@ª"—(ü¿àÃý1…g¿ä£·F4m¿æà*R—… ¿çcò:<AGNfsrq?ïòR¢†ŸŽ?R÷Ù~ؖc?@HeÓ.?B§ð'Òx?S6³°C½?L
'…Ÿ*ï?ï¤|5§ùü?‹ƒeÚã+'?d‡'CP\›?|÷XJ­¿?¿å7Ø?|k¶%Ë?î²êÍáR?–Ö6‰Ó·?—\Õj–{÷?'ø£I®E?'EÐÙF¹À?ˆµŠ7'B¬?ïå²ì`?pí¡ù.O?e#6d<?@ÒçÎòË?ir¾1S2 ?p­êzԁ?ïøbÐãå?H+ÉcÈ£?=mCsºS¾??²«™	??|;s°W?9ÿ+¹®Ë?ïà8ˆmÞf?jŒIVŽÊ?O¢­U©€?P£M9©ó?gÞÌ¢ß7?d&•ê-Gñ?ï?¾|'ò?‰¼âÔ3?‹CÛE7L?…Iß"r?"Ì…¾Á'o?|è¼rYµ8?ïúò†^˜+?Qì6î€[?	M†6Þ5?¦.g÷žµ?B¡ÏË?Q®.
hAAGN3FGL J0253.0-0125@fMþûôÀI'/`?Û¸À:Q¢xåÅÀ;ÄüÓ$Õ¢?ñŠ´(æþý@=s˜Óöã?ÿ.Î*L…?ïìóǞ Ñ¿"ÙsÌ+Š¿áê
ü™T¿æÅ&TŸáÕAGNbll?펧dÕ¹þ?±[C΅
v?™kÞe.6?ŸX\¼ò?ª_ÉÃqÉ
?ªÔVB§¦j?àv«ÙjÈ~?Ì֊Xç€`?ь}iÇ?Ç_x
¨¥{?ËUÈMP?¿¾	\íc=?èUíL…P?´C gUY?À¼j៚?® 
óŠ7?»Ú:ÍËS?¥ö"›0S¢?Ô¨ÆSA?»¦7o?àlØá-,?À¦$ÞAû^?ÄûÔ]?³ìgOxï?îª֑ó?¦§êÀÿÒ?Žymc·ˆ¹?"Õk-æ(?›'ç8ygL? ¶¡KÆ{?琇™‰?ÇÕI—'r"?Æ;ÓÚvó?Ã=pÎÊ(?»ŽÓÔEÏ?±–—
{¨=?ì?¹"V€ã?¦Ò"<}CT?±ºÕT_ò'?¡2ŒÔ–%?¨Ž¼!Ø´?–qP'×é¿?ãô.Ë?³Nª/òi?Ô®"åv?²Ë†Ï@?´À$kYÓ?¢¶ d´Á…MIXED3FGL J0253.1-5438@q— /µÐÀKVK`P¢°À:iONóÀ<
Ñ@±¡¿Ëùî8W_b@½'ÐÄÿ@"°ŸðuÉ¿âps9ÕÜ¿æHŒ'0Tî¿æ"×½cÍ¿ìUaÀS0˜AGNfsrq?ïùµ™æ»?E:qD‡?2PyI@×?=ÁrÚÜJL?@•sŒ'?7½'9Ôó?ï‡ÆD¿Äô?‡[,ßL¥L?f8AGÅ|Ò?fÙas¥?ˆ€^†´iÈ?"—ø}'e?ï,\¶e?>Òé¾jt?Šhí
æÇ?vß3Ø/?Šái•Y"Ñ?tk4"Ü?ïŒà:_CÕ?"R§FI°?W"ΨAl¥?S±¶2	õ?‰ã—£üó&?ƒsÈ|¢x?ïüjñTZd?5;Ÿ`I¹L?*¼µÉ¥?-µ³_ù ?."12 ?'veŠ©?ïؓãT×%?lš3àf¹q?T'"¿U†?S1Ä­ _ý?m#‹WÜê¸?ežoå#Þ?ï{@ßÝåh?v;kï?ƒcÌ¿Gn?pìlìd²$?{—ö¯[ç?gyMûáºQ?ïìfWÑx?aÀ¢©¯³?6ºàWŽ•{?3À£Ü•µ£?`ÂÊ-ÿK?`í>ü«AGN3FGL J0253.5+3216@bÞ>ߤ?æÀ7๿©Î›À9±€•Ó;À;*,ú4¿ø4w
þp@áܼ.@k@?
W¿å,¶Á6…g¿â
2Ì
¾¿äï«õøÑI¿"ÁjÕsAGNbcu?ïýÁðzÒ?-î‡Û?ù—û_Ü[?邶ºõ?3{‹5í 1?+#}(–Ÿ6?«q¢?‡Í«º›W?g¯ùóm•Æ?t–†DHHŠ?ƒۚWö?€MöæüŒ?ïGï a^ë?)U'B])?€…8«•€?oé;Pä£?~ß;áÃÚ?w#¯=ä?ïúéÝ·q?F{¶¶¬cg>¢I¶#0­k>¸Ú4`Ðn?DSùߤõ©?FxÐؔf?ïýøñÃÒ'?)RS ›?['•öÞe?
"B;É?)ZÔ|N?%1‰99?ïÜ¢'^k?l@*"3?QÁvE?Cõ?OÛ0j€_?j|²"'†?f|F¹ÙJ?ïªÔ'Çuþ?ožªÐ=;?qŒÛˆåáÙ?`Š²§ÛÇT?yÚóË!?h–VžÎx?ïÿVbôR3?z±‰å­>}l‹[C¡m>…k8V¥?,?d{I?w.‹ÞAGN3FGL J0253.8+5104@a¸ ٔ[ÀcßÎ\DÀ8´w⏬±À;7ÞUõÖ?ÛJg@C˟¦#@Z9€ª4q¿çEZB¡¿ç¥¼'—ó¿ç^†7Ó¿æÎæ‡ÞÜAGNfsrq?ïçØà§å?_±?§?S£àïP©?Rd6†/÷˜?\¬Ú‰V?UOp¨w›?ìt†N°‰˜?Àtk¾%PX?"¯ýß}ú?™Ì/PÍ
j?·0
qÇD?¼´>\ Î?î|Gõb?'ÄçùS?'<&èEOö?€7ɍ'«?ŸCLgÌ?‹‰yRHÅ?ìcJþ!?¤í'¸Uš²?'·kXìêÊ?…2ƒ–ëù?º·
ÔÖlÅ?¤dá²?ï÷6ŠMØ?Fi¨çOlÈ?@@eHðß?>SXã'½?Båq®€?9×>%¹§É?îêÙًÞ+?¦œwº3³…?}¹òû/	?ªfùÊ¢?›6HL±Ï?¢¤w˜7ÐÄ?ïq|Ñ!y?ynO#3ÍÁ?|Cvyeeð?i}-ˆÇ`?… ÐÐÑ?sΌ¶ve?îænâhž?"ÿ¹€Œ#Ý?yå:2%!?cÒÇâ¦?œ¸îò²&¾?"lç>PAGN3FGL J0255.8+0532@eFð¸,,ÀFÌëÿ—û4À:L‰°îIõÀ;£´©^3?Ñ¿tâ!•@
€Ý°ŸÅƒ@Ž¹?|AÅ¿Úkk9É¿äÁw:ß@¿Úo/@h¿æ÷–<ËkAGNbcu?ï·XÁYžy?yC¦†‡?;8–Ž {?A8Ô0ë°?Pü–?Ò?}Õ¼ëb‹?îù+̦P%?–ÊÖ؈O—?zs)¥cNö?€C+>¨?š=¼	lK"?"¿Ëy¾ò?îGºf˜»M?•^ÓH\¨?QáQǦ{?x\ޓ£Õ@?£[hê Ûó?Šf‰ðhº?ëú	ú]\Z?£÷Žpµc"?ˆú)5à4ÿ?¦Nô²×r?½k4ýŽ?¢s¶Fn<?ïì¾Ú›Âi?]ý²3 —?'¾U;Þq"? Œ[᎕Ù?aÅ@3õAŠ?[æ:P¾š?ﯵâûba?|âšoÿ€¢?e`Ù(¹©M?`ò)o9o ?}t¡î¡æŸ?wÇä¨Z*…?ïQ"·~ÿ1?z 7ž¬ó?€£ˆÇÅ?hqF n2)?‹–."¸ÀC?t±Ÿ{W"Ÿ?î»gG•sx?†A07Z~4?ƒ®Ù&ŒX¬?jþWé0ê³?ž»ªz7_°?'ÈYkCToAGN3FGL J0256.3+0335@e‡y¿ß~€ÀG{íÊ»{À:;ëß·‹À;©ãiÇC÷¿÷YeqžÓÀ@
|=&|?þVE^®â¿ÙÉ÷9 Ìÿå€øiø[
¿ßaœ;¤4¿Û%¸«6AGNbcu?ï§<ϋd?b®ï—?9tÌÁ¹µ"?5Ó¡Õ3Âà?…e%®Qœ?€ÑêÝEÎ;?ïˆ|í«-…?‡^ù›îÑ?cޙ1KÔ?eõ>Aïbž?ˆéIé™f?")ÔàЎp?îm€(%ÛS?‹xìÓ¶:?º8i‹±e?zãKþ~ö(?¡9oeÓo?†`é"%"˜?îހ,Fk0?"ˆ>"HoH?(²>Ãó˜?,/Ÿ±ûBv?¡ÿK4'Ëø?"vvx&8?ïéÓÙ0ˆ^?cvÙÐRQ?(NH^ÿÄæ?#ŒŽSi?d§BSÖy›?bږ¾º¼²?ïØËÄË1Ó?kôüä)[?S¡Öž™õ?R:`Žël?mcP:Ím?e8Æï6?ïW¾SžsÚ?yú}/»ºm?€æ°ý§?p‡f§­?‰r"d¥²\?q'ÝSym?ï¿P…S'x?p-ƒAx¦F?°†ý-Z?•…a`?€.%í!n?p'QA·>AGN3FGL J0257.8-1216@hsÿ¬*ÀLr 6×-À:¶'Τ=À;ߎ¿K
?ßғ»‰-'@WðK'	…@Òýßê5é¿Þfé=¿ç;æqÓEÒ¿è\+´d1¿è71¹¥A‡AGNfsrq?ïýªs«?'¹RÿDÿ?‹Xãzñ?xrþÕÂ%?(Öùó¿'@? <_ðžÝ?ï‰ê;¿ì?¡"=Rÿ?jåñÚK/?¤ôf"څ?†ËôŒc¸þ?†9T˜F°?ïŸï	Ò?'<'¦'É?‡%΃¡®¾?v¾áñ,î˜?'6`MîV?x(\»™?ïby8ó]þ?Š~Á9Ë?aƒÉ#y°?\hqìG
?'€_»ñ@?‰‰wlÛæê?ïþσ¶Xl?nr+0¶*?ZÏ7ß?	ñ›\>Þ?â"Oo?ЅW7Á?ïܟš(y‹?n`ñ=ä¡ß?Q‰­0k€?RU¸í¿…?j›ÖÅÔ÷ó?h<6*I*Ç?ï™6¬g?mJ6-µÖ?vÏáí)ë?cšF¦ü-`?|Õ(š?^üåOÝ'?ïäwܹ¥?aGñŽsš?JOº`í?:Ǘau=d?dô\~rŒ?_=EÔ?«AGN3FGL J0258.0+2030@cßdÀßXÁÀ@¬‹ŸÛÒúÀ9úá:B.À;{E	õLH¿õq.÷iÐ@'Ý/p…ú@!VÇE¤¿î[r:"U?Û¶æˆñ½¿ä]}«ô²¿Í.–Ì	ÙHAGNbll?ïõB'
ó¢?UÜy~Î<'?3e0
¨³?5É;œ°?P¹"ë숎?QÜð{fŸe?ï†!{6r?ŒU€ã)?kiZnVæê?–øéWe?‡J'Æ!Õ?'Š¯^ä?ï	˕ëV?"ª">Šø?†ÿöø#¾?uÏíoÚÛe?"F'5¢#V?}ªê\O@@?ï"X?À…?"õ2£iœ¿?9+g3Ù1ó?@Øù°èÔz?Š`"àåB?"ò;»$Ö:?ïø¦èÀ%þ?XuO•ó?(Œ(ÄÑ ?2l°1‡P?GAR:Ýú–?T f¿2Ÿ?ïتÆ"ö?l« ŒáX?RÇ\RÕÆ?Qb7M	K@?m٦њÏÀ?g7"û?ïŽ=Rpæ?v<Ü:ç$A?z
yÿåß?rF+ÕCs?~ÓÜáÄâè?d£†°;z?ïäâèÂ÷Œ?^®\ˆçѨ?
ÇóŸãœ?
½bøcÕå?j±÷I{0¼?^z½ïÇAGN3FGL J0259.5+0746@e$»%_5ÀE§ÒàD²À9E<æÀ"À;qkI$6@?ÙzAµ,>@ÇâöYã÷@²v BÀš¿â9˜/¿¾Ð¿å?U÷i¿ßK|‹ýàÒ¿ìfçsI×AGNfsrq?ïó‰«ÿ'Š?P`:‡?=dœÉZbÖ?=$ŠV$§&?Q"€Ú@?H'.&ïV?ïmø1¬ò?Ž'
~ϱ?n·øצ`?|Ånòl'§?ŒÓõlˆ×?…Ü"*LYË?îwc6¹®?"p¾ÑXïþ?›ÓPµÕ-|?Á׫lÀ?•@Hvd«é?ƒ{ƒÕrC?ïËÓ'¯Ç?'2°×MÚ(?]¤µ—×´?Y™ýA´«?œŒ:>ù¾?'±¯¤˜²0?ïúA&æÉ£?:FhŒÀÊ?3ÝÄ ršf?+ÕÙW¨Çâ?:n?ýK?1AY˜D?ïÍ{)Ûµb?rñ·ò°ñ)?Y£çìYû4?WC¥ÉŒ&C?rÙq'Œð??mò	*̶j?ï.טÐt?Š'Í
›u£?¢ŽÁÁ"Y?†…Ì`ªàu?ƒüT'C?uózQ#	û?ïÆÔâlá?l}*A)èr?R&#]ò®?C¹;GZŸ?xv°1rÖ?k5­Ù|AGN3FGL J0301.4-1652@i~à°¯`ÀM"€ŸÍAÀ:Yx°"À;ßÿê0Šâ?îöŠâáP@*³In@4`BŠê?îÊ«ÖÊ+¿â²W¿Úv¿ä¼G_°¿è$å?èÖÌAGNbcu?ïºH@5¥(?z˜þ?tàì– %U?sk5q!?kõæ›ZÜì?fÂB±ˆª/?îºîœýb?¡|^¡%H?‡ò5¹‹­?Š‹(÷÷Ç? EoË¿Ü?›xªX-¾?í*0Þ¢À½? vQ{SА?¨×ô??˜'þv½÷r?¤"þÚí?'h\ò³ü?ê¿óܗV?µ÷0ÀR›!?±?âh‰d?¢5tcÑ¡ù?¾Š÷H»?²Õún>Χ?ïáÓ7Ü Ž?f‹…ƒë?aSÎ6½­?^aŸJ:8D?Y²t R¨¿?TUdÉ Íá?¬Ï"à?Š
óN9ö{?t"Ê,ï*?sàÉ¥ñ+Õ?…TÖú¦Ž?ƒŒR…r>?î¼K'p²E?3ê	Àë?—º…Oõ0¥?‰ð Wòú?¼ìTÂ?ê5»;;?î'œüûhÂ?šf"É®ŠB? ô9J¿åà?‰²o±ò3—?™#í΂¸	?"öë…AGN3FGL J0301.8-7157@r ÿâ£ÏÀDߏÿ¼ä!À9©&Á½¥À;ìAVâdå¿ýÛZY<Ý+@ѾÎ\nì@ -à
q¿æþ¶"Ç¿ê¿çd…'*W¿é9ð¸Jšê¿ïþ×;ï"AGNbcu?ïûÚ?ëÂ?:õDDI?!c—Ô?!twð!·?8¢N±M"z?7¤¸íy8F?ï»p»¬?ŒNœd2?jºÁø''?|NÙm¡C‰?‰Œµt#,?ƒã5Ñ#í?ïçcé?'|çïÁ?
×ýàô€?wÇSÃî?‹;c…å0?u͝bí@?ïî—yü?}¤¤¸Ò1?9`J1Žzõ?OAM3ã"Ã?|æ#÷ˆ7Ÿ?}`C¼q?ïý+îàÞ?-÷ò峏‡?#M¾rs? +¬õ÷7?*@þ°n(?"ÒÃ¤U?ïÚ§Ý:io?m.æe®¿H?Q­[Íñ
?Q`}HÌÖ?lt¼Aó–?fºörwë™?ïb&-f?¥?s8CÑ¢ˆ?‡f[—åÁ?k ×î²Þ?€õMïÖù?f¾‡2Žp?ïõÊÏòq!?a	Xéá€?±Úkg‡?9¨ØÏg?S¼ÐøJêã?`đ&ôڊAGN3FGL J0301.8-2721@k =ÀTïFÀN‹_ !¸À:ÃhÍJ¡À<îл?Í°¶h)@
`+¾ß@CA¿½ð'?ßóä²áX¿Õ¡ Á"–û¿çšS|:p¿ãºØ0AGNbcu?ïµðéGèÞ?¸U÷ÏI?sÅ Z–`?€@@æ8Ô?qAêégí
?lÖù"J•–?îºêïo?±ë"5¢/]?'ÖÍ݇? x锼b?¤™Oêönâ?¨©á/=,?íf¢l¸ T?œ}Φ°r=?¢ß:%ªYf?"·«
Æx[?¦¶ŸÓ¡`?'hþ°ÅfC?è'éZæÅ5?·ŒâýRàÿ?¹õ!rÉÿœ?±m?Ïû`?À¹ÉÝ%¬Ú?°¡ùì=öô?ïéÜ(Eª•?bä -P}î?Kƒlրk?U,€Ù²¢û?^…ù»'¡?Yÿ''[ç?ïƒ+›†¦?'|µ< 4â?r$$ëNoˆ?zæ.w։?†-¢—ÈrÆ?‹\î·fØ?îσJo1^?Ÿšî?"+T7Y?‰$0ìß?'kXë2ü?ŠÃ]±»?î9lH[A"?˜«sÙ
e?™\Œ˜¶7
?ˆ†i%(?Ÿuê_Q@²?'s˜S‰SAGN3FGL J0302.0+5335@aµt!-wÀÎëÿÂîRÀ9±ôafLÀ;RN©±>Ò¿ÕáVՂ[˜@­Sk7¦@'€L–‡¿Ó^(²Ú:ý¿çl*³e{¿ê½·õ¾ø¿Ö—I³'_@AGNbcu?ï›.Bò?‡»{Ž
@Ó?(mµÏ«?"Ú^øâ>?s@…˜9)
?s¹çHuN?ì^ګݔ?¿Ò|Új£?Ž¹ÅçˆîY?"Kû‹dG?·¥Ðlf?¼}·`?í©ËC=u	?šÊ°p¥f?Ÿ‹ú¸æÒ?gÂôâ?¥Nè#?'žWOêp?î)¿¨2Iå?šïò	ÕéA?[ånÑ9Y?^¨w {A?¬"Ú%›á?šÄ0{ZÚ»?ï×-;ï½?uVäήFÍ?e °<Þٛ?q4=œ;Š?cÐ"'0)£?b^­ŒÏ'?îñI$Gn:?¥»A¦fÒ4?wpt©Ä?}LÉ«¶L?›ú¾uç¥Ñ?¢µöíÔê?ï	;
  }?ŠátcOÒ?¸"Äc?í?'£)V5ÏÄ?ø¨ò?€¦‰â¯q¤?‰W'?t~;…—M??Ø~¡'?3åo¦ºj?‰&ÖޒÆ?t%¿-AGN3FGL J0302.5-7915@r|>KZÀAýVÿÁßÀ9æêºô]À;¾˜Ã°ÄYÀÆã<û³ë@:Æ¥k_@R_žK/¿âß
e²ü¿è†BPÿÄ=¿Ùv?/Y¤¿ëæŠx
õõAGNfsrq?ïû?>·ÔK?=áO=f?¯)'¡â?ŹΦ'??ŜØóW?:91¬‰h·?˜ïr?…ÿ%hۑ?fb(œ\é¤?fnՎ#)?‡8O©jÚÛ?'Ÿðl*rà?îý[Šë+?‡rÅEf^?‡pP´ž8Ø?sǘîœS?"œfAlJÆ?"QªàÈf?ïÓ
‡©"H?ud¦1%f•?}‡ØÌÝ?R˜ä*Š?vV¥.ra ?uHÞõP?ïüÀ">È?/<¨…ÿí?'yÖ2Á?菶\
?49¡#]??)¡""2?ïÜѐ'0?lFK½½k(?PÏ!Ÿù?P˜Iå?jÆÞóTCÏ?f®ô˟ ?ïõÍ»Îç?u:zz?~¶6ÉBç?fÉ8EÔ9?€§q"Ëê¡?pGÞ{ùÞ?ïøÙ…'?Lè>òÂ>Õ«ÍÌFñe>äü¥{´â?O½EŽr?Kö|¼È¬"AGN3FGL J0303.0+3150@c"CŸý`éÀ79՟Ú%{À:1æÒ1œÀ;ª²²oSu?ét4'®ÃÍ@
š{'pÖ,@…¿rÇ¿Ú¹éï¿åsÍl¯Ö¿Ù¾Uà *‡¿ïÿÜBê}AGNbcu?í Q$Œ}?²áŲp7ó?Ž°k?'yìËúþ?®NÒÅÇ?±dM*>èª?áû¡žË²›?Ç£'ÜVÇQ?ϦʂxHo?Â`WªG"?Èj¯Xí#?¼˜jQyçš?è_·nt=?­vÏ ›?ÀAItÆÉ?¥QÎ(M7?¼²Š"Ї?¤ø߈èÑ£?äÓ¬?¹ŒiI3"q?Çؽ#•?¸²&¯÷fð?Ȟšw"?¬êûõ¤õR?îÿ¸'~?¢Ö€²piÅ?túG+¨h?|撈eº#?šÊ]ïén? æ¸l~¿Š?èã¥P~j?Á\{ê9͵?Á$Eî?¸oHiÿŒ¸?¶´§3ðyN?«ÆuRo?ì-L@QÁ?¢bâ±è$T?² ÞƂ,?šƒ"Óe¢"?¨é~n¦îð?"HhÙÆ ?éÈÄoä?¥Þ°&³Nö?Á ø9i.?£îþa*£~?®ïØÐïC?'Ûy2ÒØXAGN3FGL J0303.4-2407@jÔ5 ÝDÀN‹`òËÀ7qJ½"sæÀ:¥C'&Ò¿ÏÓXî@ÞõCc'?þ±Zá"Z¿Ø,ôˆ¿àÉÇ{C)¿Üs,aK¹¿Ým8<²béAGNBLL?ïü "ÚÅ´?=åÉǤ²?	^ñ£olt?Iˆ¬y@P?;ÏùÅí[Þ?<Açdõ†?ï°X«Îâ?ƒk6ôw¥m?_NuqWÄU?cʕnë?€Û+XÍ?€¿`?îHÓB"í?›ñö4éÛ?†Î¥¹^?ƒJÈÛ"?¥ÏX,ؙ?˜©²2Æ"?ïäm€('?j狄uø'>Ôs®&ôT>ûŸ¥v¸¬?kˆEügé?jâRä2'ó?ïþnºÃÇ? >|r`/H?¥ÕªSG-?6™N¢µ×?#j눡€…?p6wQç?ïåDž˜¹R?hgЩe;†?Iì^F"áF?N'.A°?c½bÙ4€c?b¨Zoì°Æ?îí¤ž¸ðÕ?"ù¦fßò"?'4ÆCŽO°?€¬] öà?™1þ¯²†?ñøc%)µ?ïø—û×Ö?J6tœcg>Ä—0Ïè>Üâ|¹HR?M‹õÛj?J4ÜSîäAGN3FGL J0303.6+4716@b ŸDÔEÀ#¶î#;nÀ8SJM++þÀ;N"šVWû?çÂ6oÂts@å-oÏƧ@D¦€1釿㞎ŸÚ?@¿ä¯àWæh¿äú"â?¿ããœl²°ÂAGNbll?ïêCa?]ü
Œ†ª?G1ÒPÙËu?F©×ò"ÐÇ?`'HŽýõ?X'³+³÷?îœI!勓?©"iඒ
?Ì'£ãŠ?‰ÔۙVCR?¡ÈI6Sï?¤š†éé",?îÔ·	õÒ?‹UH'dˆ?ŒŒïöxÊ?}¬['?øO?—"§Bü3U?'{ŠDNÿç?‡?†n:`È'?P½ä^½?P ƒÄ?‹ãWgjÔQ?…÷ã';Jg?ï÷qª«ÿ?G?CÐû»?9Éá¶ë?6ͨñÇÂh?F¹«),E?A–¿šY«?ïy´¥ŸÈn?—cĬŠ£?jhs¿éÝ"?pD".¥Â¸?Šø¹§»w8?">½SRÐl?ï‡ܔ@?týÕS:+ù?ywjž)N?j¤°ŒñÞ´?|S"¬¸ˆ?jçÐoÐ×?ïäßØd§í?hKp 6r??z(
KŸ?4.=ä!o?g0âÀéœ?gOØxY/€AGN3FGL J0303.7-6211@qƒÄßÎ1QÀHZ$™ù;À9!ý¥²¬À;´Ñ¤¢â?絶"ï̵@ëxˆ§Ú@®ZÀr¿ä8ÚSÀhÞ¿çVbÔ¥M¿åD'â7†¿ê€?(ðö3AGNfsrq?ïôÑ®D?S@{W$?FG¾5æî}?H*ŠŒ4°?I@ýákº?CµƒR5?îúҕÓUA?—"P±·?z9¾CóKô?x_|Þ<&È?š=­aVð?"ÑEÅk‹h?î󂗅©^?‡w.?…?ŽUؚ»w?{û¬\â}'?'e"$µD…?M•¶þâ?íޞgÎ_8?¡•ud€U?‹ˆ‹O5®?}S©®v?«3ö­"úÙ? Ou}î]å?ïúWo'«??èº)Àû1?8Š×}E-Ì?3Ötz'­U?4¹®††Î?0˜f(?ï­!g?œ?yeÿ2*—ª?f¨'"&•?`le#³Gò?~I‡àk?to³KÜIZ?ï?âÝÊ?qá[}ëÅa?€q^›ý†-?j'ü'•"?}QU°P2?dN©Ñ‹% ?‡xYÙ?Z'¯"ç?uÿ.ñE'4?a2.nø»?ƒ¨>æ®?zH>%;|AGN3FGL J0304.3-2836@kõ¤€èȬÀNWþKZÀ:òº.d—YÀ;æÃ$º?ðíÇ¢@gËOKE?ù½AÑ6>¿ï»¹/7Å¿Ý㔏nm?톣Ùʝ¿ß…±">jAGNbll?ïÊ_6ò/ˆ?~û®_ïìÇ?U²·O"-?Uj^ˆ'Û?uc¶Æ>ªî?|N–ÝBãð?ï/k?5—^?¢2ER"¢i?|c0ô?Šót--ȁ?'ùԏ0V?˜Ö@xL4?ìÐé5_?¢Ôò0ú?£€Ûsãå^?"z¢ÆY?¯pŒ•[8¹?œ±‰zdz?î&]~ؚƒ?µð[æ¦TÍ?p'Ñ—ÃpÐ?Œ·ðf•?«‡íàØ9?µµã*¿ï?ï×Ô"°Õ?qy:
ò?Pc׈mu?IÊìPÎ?oùò_/¡?o¾5Ùvk|?ï¢2?"§
ÆW'¹?oÀŸˆ?€°šÀ¼¾?ù7¾M"?‰Éi™`^œ?îr1†hm?•a¥qè=?–Â\´Ët?†¿ä…Eç¥?š÷ruåk?ŽõCÌ"?ïrIšÂ}W? -à¼W"'?†ú	å¿´?š0¨-Iþë?æŸFÚÂr?…mH?AGN3FGL J0304.9+6817@`Ù´ßݵ@!*ŸæºµÀ8±ÕORM«À;PgžtÊ­¿àiÐu›/@‰7jöC@Á`)áP¿é]£G©s¿ç5¬âC#
¿éÞ6%DÌÒ¿ãQj͘ AGNbcu?ﲡ1µÒ?svêJ³?x¹Â8´#v?zAż€?këIÄ(P?níáÔ´~?íYʔÁÌ?¼«ˆj®ZØ?'2þ¯óÎ?šQ?gèÕ>?°äë®Ð'ž?¸0¨7™?ìÒyßaqV?¥æp­9"? úäM¢?'7Ã'ìßæ?±]3§âÅ?¡¬ymš±H?ì')ô~'?¬Ê½ÑÎ?ÂýL8Á&?7Ø÷aýŸ?ºÎP´½%T?ªMžx¹j¾?ïì~µé?bç‡[OI?WŒ ¢öYJ?Z ß´á¶?Nï¬,²Ëp?RP;¶HS¼?ïH48tn? fÆÙN؄?vš5ö­?€gÂ51ù—?'w2ý³h…?š¥˜õ<ª?îük@?á?ÐuºŽ4?‹qZæIƒS?ƒՔî'?'¹ê†–éƒ?†¥kiB?ï$Õ¡Kƒ{?ŠO""†…!?`ï"ïb‰?T\/¹%¯ù?™SMìX[?‰ˆ±ÆµQHAGN3FGL J0305.2-1607@i
l <K
ÀL'BàO`À:Š:¶µ3SÀ;Æjd!èˆ?ç·Uðêc@
x¯¸k?û!Û­?ïºSzÍR¿éévÉ¿º6'äÌ¿»Téj¬
#AGNbcu?ïÎjÇ7#?'c©_ľ?,}žÿ‰üÊ?3;¯Šü¸u?wæ¯s3÷ÿ?'MƒàW–?ïŽYf›?Š
"»i?g€bŀÕä?s/E¿‡&ì?†‰¡­~?"eå·PK?îDQènؕ?"]ñpò»²?‹iø­?y ²Å•?¤àœy¨Š?ÅãÇf?íÂÝø]Ê?©¿Ÿh•´•?c9YáEqN?uBÎ^Ôî?±OI2É·â?©KiŠ-õ?ï^4¸»À,?¿Álíû+ì?=
÷ ÉÌ?tn…¤Y8?"Å·"?¿`^ºu‡A?ïÚ]-…Ü?nÕ¨mcÝ?Q¾zkÚXK?PsùA´{?lÕާ[?hèQn¤ÑÆ?ï;¨™š	?ƒãô¢Ñì?€#"›=º?qr°'Kݝ?ylš¶cÐ?6Z+°ã?ïŽÝ¼;ã?‡KÇ3Ë?`ôh&?éÕ?cŒpoãj"?ˆvØXÙü?…Ž.½"ÚúAGN3FGL J0308.0+7442@`w¿Â"O@,o[Ao6À8ó¸ÒDÀ;Ý@ï´Xb@H² y@\z-m¡n?èh°n$ÿF?ã±i¸"A¿Ò:…ÚAvå¿ç[ooyŠ…¿ïÿñ­µcPSRPSR?PßQWã 3?eø†	Rà?ï¤`úìšÈ?¦{zÌYG`?"Ë×+
õÆ?¥}5ñåœ8?fßóT§ËV?"§×g2þ«?íÙ'Y6'?´st'®[?°€|PÙBn?´WT¥žµ?§,òÓ íÄ?™"!Ò¼´?ë:KwÄÿñ?«0ÛF
›ý?º—*ص}?¨S4ËÝ»<?†ñÔÏ^,?ƒ©R3tû?ï,Úß½ã?•þ0ܑœè?×sýzU?'+Bè¡®U?GK·_Ré?fgî‹ïN
?ïV–úõï?µÁ ý±´'?"tEE[3??µ–ömhX?uýr9¶ãŠ?†YM@~	?í‡Øú¶»?´ö9×Õ?²aaX™1?´'î6Û?¯?kݖ"? ½bc±Ý?ê¢è¬ôŒ§?«øddµ_"?»I§jμ?¦p—ù£é?¢J±³y''?'Ûb'A¬V?îz¾¦Þ?—kÜÕ«)?ˆ%~4:?‹°0ˆ(ÆPSR3FGL J0308.6+0408@eÜ:Ã.¾ÀF;à0VàÀ9¾Î?""ÆÀ;#†Ö?ÛÏÐÄsq@ðE®_ú@'‹ßǦG?ïðBÐ+ž¿ê,²€=¿Ì¦†iр¿â¢æ1ð
AGNrdg?ïöœ±üçÈ?Kh-{H­?.¿˜ØJ^L?)º§¨*é?MÝRÐqØ~?H¼­/^0)?ï'au]F¤?˜v±WéZ~?uã6e?srîŠìë?•Ð؂à?•»a®UD?î´v¦òÀ?V¡®XF?ˆ"/h'?w<)€NJ?3ÙjLÌx?Š‡,`"oÔ?êñ³ ù+È?²¡øzö?wM=ç¢?'Ó¦*?Ã!¼¢L	ˆ?²E-'–b?ïú-£?B¤|70?&TüÄ6b?#`.Š6¨Œ?Bn1×ûº?@)üƒ1?ï°4Ù% £?1qƒ¬?c¬Òi@vÃ?_³œ/çv?~*9ïJà?}y\}{v.?ïm6È¥1?zqÄÇâ_?{•Õç|'?jÒ_ÄÐÆ?†çc^Æ =?tjŠø>+?î'Yߪ?",(9öj?}ÐÜp˛?l;ˆ¾ÁKƒ?£$8s­Úk?'ùvNXAGN3FGL J0309.0+1029@e%F?ÀCێÀ!ßÀ8kÖÛCˆÀ;-T®­ýÕ?öÝ7ì*‹@™»þHp?ÿã»(Š¸¿à.–PŽã³¿â]ÎUŸ*¿æžƒ8â¨4¿ä
(|Bh'AGNfsrq?ïøã-{'?Bä"¼Å?0u¯"(èÌ?+íDk9?G±›ûþ‹?>4®Òw?ï"S³u&·?‡†¾fþï?eYøÕ£dæ?sˆ7¯·BÃ?…""ù¬Û?€ÕkU,?îtT»™?"æ"Š¼ý?•ŒYF®«?Š¹ÆXì	¼?˜Å$.û™?Š¶­VU?ïÜ盞ñ6?sÏä:<V?$
ûiXO»?1Ä`øJšŸ?pëÚB"¼?s–2}FúÖ?ïûÿš õe?2KfïvÅ_?'&/g`q?!2ÆdOS?4p`p5?)u4÷-·?ïÚÖj°M?m.ƒÙÁ&?S+6údøå?R—Ç‹àŽ?k"ùÙ_¬2?fn)5{àh?ï:@^žz?"þt]^Û?‹N¦A%??±Ô,?†cšY2 d?wÔÒås—f?ïøª ùU?SÍ?=ÐöOùU?.'[ÖÕrË?IÆX'³ä?R*â"õÌAGN3FGL J0309.5-0749@gš·?1n7ÀJWÿ›V2À:åsŒ¿—À;¬Æ8^_?Ϥ'౟ä@Lªhö‹?þöý?†RÀ¿Õ}¥kΞù¿âéC¡¦"?µá݈ºVÜ¿èœ)×È\AGNbll?ïÓ©eß?tãOä¡Ù?Kìĕ¡¿?N
p‹
«?s­ø8oå?rñ´ï¨W?ïKt—W?–¶É˜IiT?}Ðea½c?€s¢3ýûœ?—ℳÈ2Î?'ëUJ 'P?îzp &'?"ÓYš*W$?"<	òkh?ˆ¢íÏR˜f?uó+™&{?Œ&ÿ»e
?íq9C¡$?ª#È#s6S?v@ÅÇdÍô?{ÕÈL&¿?³)…™ä@?©U1ؼ™?ïÞµð'NÍ?"©õà«÷¡?F àމH?qPH®vË»?k¢	̧Îê?q¹¼à×­?ïÏøÀ?õ"&lݘ?nàc•Ä'ƒ?l©º£PcÝ?€Ô!ãü@?x•Bz)Ž?ïG–õÄN?…–pF%W?"›7°[Ø?vX—0á²?‰~á‡nôª?|=Ç]
•Û?ï=WéÝ?‡Û\¨Æ?v½úK³ü'?o+–Á€óð?'¯Ösžñ
?ƒrññÒJAGN3FGL J0309.9-6057@qa¦`ɊÀHyðßьOÀ8Ÿ' <¶À;¸éÀùZ?èªXðeÞ@׌yËs@_žŸ½Êü¿â!©¢?h¿çÚñA
¿ä;Ýòö}¿èb]{AGNfsrq?ïúOFº#¨?@"ÆÔàlµ?-/¤ƒ³û?0(¯U—ÌR?>î<ÌRs?6µ~
zÁõ?ïz¤gí"Ü?‹Ò­,5¢€?iXl@k¥?sè:vÜL?‹ËB,?†0Á±H?ï
€ï8e?ƒ-4é;?…uöì,?r%Ã6âœm?"$Â/¤ƒ9?~<·EŠ?ï|'D2+n?ŠeG¯ |h?UžMÉª?Xˆ£™Jö?Ž'¥J!Ã<?‰Ï¸¼(ø?ïý§8ú®™?*À±–?ÐT#r¡?߄†ç›?&$C—wû[?!1—5È·è?ïÒð©\'?pZ<ý}—?UkÁ2¸V?S ø{ÛÒQ?q,é°ås?j#¢²Í?ï'Ho«?sÚv…LÃn?vñg–$4·?pô€-T|z?ꊻ@ñ?aÛ»PnD'?ïæ"E'?géU=Ñ÷?CqhòƒË?92ÆiAö7?dŸuž¹#?fËõ7Ø:AGN3FGL J0310.4-5015@py'ß֔ÍÀKr<à[À:3maÚÀ;»€šŸS?ìêjûݗ±@õ;Øbç?üÈ>Ï¿éFчƒ?Ö[4®³\¿ÒÑe™žy¿Ö|뗬ô.AGNbcu?ïùÿ±KB?DÏ9má%¬?*eÍ͓•n?&ïw­^'ƒ?Agǝzø|?AöµFž?oë?ˆ-œrcN?g¤ Û¸,?k+íçøö?†î›ÑºP?"JÕB&?îÎæÍ©ìx?'m"Þ `'?V­AßKê?†ꕰaú?•Ìy

?Œ§d4<Z•?ïi‹Ó2m?‹K	IÇø'?i*ƒÒ¬?l¸NK¯Á?xÒ_ïåè?ˆÄ[96­f?ïüÞ`P«G?0$/àê¹?!¯ÄXZÏ?c¨z-?-?0Œ¤ÝŽÝV?)dGlš?ïÖ^~îûÿ?qÑD¶sÕ?T5\ö«Ž?R¯%ƒìå?o`æ5-Ó0?m¥·Ý˜÷.?ïhþ@ã?‡¦÷Ño
?'8œeþ/?»‰NŒñ¼?ƒ‡ÓAÆ-?€3…à̀n?ïϬLñí?h'z{>¸>?eæ[Sä´Å?YÌCYUåš?jmW¤0;Q?at°3–ÐAGN3FGL J0310.8+3814@bÝF€"À0ñà18‡À9›á·?œÎÀ;š­•Ïà~¿ø´Ô2œµ@cÏÞ$8@c x›r¿èÖÚJlh¿èBxŸñCò¿ÖŽ*ľz=¿ékë-ŠýŸAGNfsrq?ïü6áú˜?<'sÞ½ ¢?#ÿ<'Ø·H?%ˆ‰\"'É?5Ϊ+™´ð?5}6©•†?ï~fƒ¨Ò®?''^1¦¥£?nÛØéú$?~P4•:E?ˆ¯œ'?@Û  Ý ?îú°Ðm#?ˆ	‡¢¨	?"éßÁ¢ö?u…­9mº?–5`º"??…["²K'?ïÎ5¶	+?sµ#›å?	nÁa?}Âw'2?xÃc5:9¯?rëJhîÔ?ïýÂaþ'…?)è't|?ÖˆÜà?Œ<5/k?#îÚ[L? zËÌb+?ïՍLš/?qMÛ¹ÒZ?V¾ç·Tڔ?UÌ^ÔÕçt?ot«Àd?jX˜›¸oØ?ïŽþõá:?v­ƒÇMnŒ?xÛ´®·OÅ?r5Ms·?¤Ðišdy?g©Dvp?ïö(ÈÂ?MßÚ&ÖUä>ìŸÒq©>ð‹-"¦¥?Sv°ó"Ã	?MÂѦÀ$AGN3FGL J0312.7+0133@fP†þ÷ÂDÀFÁÿÑÀ9$5Ý1žÞÀ;×xø?ÒSDܺ@'èá'*@B¦@#¿áëŸè,œ¿ä
ÔÝp¿ãÁ&~¢zò¿ãÓgTmãAGNfsrq?ïöÐu	'­?Nú¶Û_?%ÖA‹ª´?#IÐo ?Oyö<&w)?LÎjŽ¿?[ßWr?ˆc¢F½?eà™ØÞ?snúÉ/?{?†°þao?':eå3·B?îþ>ˆÀ-?‡~÷€b?‡ÖñTEÆl?uR‹F|\Ž?"L¶52q)?€®gbãð˜?ïÑÆàéS/?qûÊPÛ? Å5³Ù?"î}þ¢:?v–gã·Ð?qÏoø_?ïý:Œ¿/?-5"‹cJÉ?&­á)e?ð·#òw?0áüC»Ì3?(Å>Á}Çó?ïܦUƒƒò?iXRF/Ïz?QFþ›î´Ü?Pv#»K'?j¶+N!?ce)N|À"?ïœ<|7'?p=0l_b?u<2÷Ö;?d@MÚGÄn?|ۅ»­øò?eÕãnFQ?ïøPvî|~?H1É>Pt?¿©i	Âæ?Q6cP?LÂ*1;yÌ?GÑk{œüAGN3FGL J0312.7+3613@ce`A‰7À2mêÀӚFÀ9ö"ö¥
kÀ;œ'«hÎö¿¡](þlR@Pà$ÃXÛ@E"…á׿ä'
Õ#»ú¿åàÆ£V˃¿âÑz­Ž!¿ãRt‡ï×AGNbll?ï躩‰¦²?bC9¡‹6?=ÿ™Ñÿù?9ò›} ^?c¢6†±ØÓ?`YYðÊ?ï1¸7¥™é?™SÓA»I?xJ‹-¡?|	™Yte?"¶VFfIi?–(K:Ë^â?îÜAÃހm?Œ<wFáÐe?ˆ¯ûìÜ?u´Ã²Äþ?˜ɈšyÜ?"–Ý-&±?&ëd?¾˜{¯(?hQBH=??`‹¥o ®P?¥ß)Wƒ?Œº=Æ7›ó?ïøðŸÃ\ê?CÜÍ辜ü?&/?ƒî/,? ÿ¼ˆÍyA?F±²">—"?A€ß8CÖ½?*µÙžË?~>ue@¤E?`>!ç`'?Y™ZSp?y›"A}:I?zTJX=¨?ï–fU7?m܎a.O"?umñk+ãÚ?`KÐ:!i?_Ô÷lÌ?c–ãåJБ?請«oãp?j랈
5?W§Lí9ðå?AÃCnvÿ?'\+"ÎA¹?hØzšæAGN3FGL J0314.3-5103@p…B 6mÀJýJ 7BŒÀ9˜0P)ãÿÀ;ÝÕC"Ó‡?Û«Qß¾
@oŒhC5@3üu¼¿æô ¦ò%U¿ãžlO'ì¿æKr7#¿Ù©©1£LAGNbll?ïÆ-¯CW¡?wM"BÿºN?hë=2]óÃ?jåɞž)	?ps‰Þ'Qd?m½ro¾¾¿?ï7Ú~CÛ?›æ—ûÀÈ?vÅ×\=-¶?'™z㿎;?"nNÑÅ2?"ý¹Á¼ª>?î/<'<s¾?"èü–.¤/?•ì½&=`Ç?ƒ›•L"?¢ÞùõúÄ?ªA,|'?íÑóÌé?£'z"qI7?ˆˆšNèsÜ?ˆ*˜M÷×(?¬Ìz,ñï?¡›Ô´ÝÑ?ï]~?^î¹wؙ'?N"JUÙ?NfpóO`?RЄù·¯	?TjӘûÝY?ïŊšï?{Š½–V0?^k¾È…É?däîðK̙?u"•¶òƒ2?t¼°O?ïYÓÑ"òÉ?x+·'mÐd?'·YЃI!?p«ž¶l??†Ó±ðö…?k¡ýl{Î?ïFŸ+?€'âPX¼;?oþ…¬$Õ-?a›
0PAñ?"®¶ÝlD?|Œ®.fÎAGN3FGL J0315.5-1026@h7¹ÀëíúÀJ=Ÿ¿™À:@¬˜yßÀ;¸­7Ü`À«Ðo¼@ÔÓêÎ?"@GÑ?Î!6¿æfݲMD¬¿æ™¡Ž|ýN¿×"U0¤¿ê™ñùWlAGNfsrq?ïþ4Z>~°?'hßdÖ?	¸\·Ðàœ?}颉5l?&LH—î€?$9ÚKƌ>?°¾p¶?‹£ò{'Z?eå½'BÛ?{½<éÙ?…™Ëî€{»?'fuÑMšÿ?ï¦òau«?‰tÛ]Úä?"}mIJ»?wÅ«=	 ?"jÐ#R?" 51h—i?ïäžb)‹?g1#?ˆ>ã¤Qðé1«>ñXû\A[{?kMù<×H¿?g)ÞVÕ'N?ïþ×à7sñ?~)ï'j¹?
HK)e?ð®*¼_?ßÎìÓ?"â—ðÌ?ïßÕXË@?kfK¿–5f?N=/¸reõ?P${×ó
?h›§·þ­D?e½‹(Ïm?šFt?tNÐ9í O?yX´¾k?f†Ž3$ì?~"ZF|?oËá¨A¡7?ïû,î9r×?=֚}¨Æ*>Á$&Àš>ÉKìEhË°?C;"Y™A?=Éê—ø¢¾AGN3FGL J0316.1+0904@eƒ  ôØÀCÌ¥ 8LÀ8aCRe'¢À:õÍêÙþ?áØZx2
@°¡€mΐ?þ©; jM?ßÄèÅÚGè¿âÖ¶ÓÕÞ¿ÜR­Ÿ¾`¿×ïNBßAGNbll?ïÎi‰ÓË;?"V'H@…\?0/×êPV?0öÃÛ@Ú1?wÈ=ƒß—,?"$[ïös?ïM|hŽè?•im}…2?p]шC"ý?sÝƜín%?'GÍyû?"& íSÔ?í°^F~¶â?¢'a.+'?Š<WÚQ?}³q½RF?®kÎÊH¦? ýc¨ÒäÂ?é™Ñ}¿&$?®'Ð-œžÆ?vÚõ:Dl?w<¿~Ï?Èä»1€î?®{/"nñË?ïö.TžŠ<?UþÕ&ó=?ª÷evý[?|1MjQ¡?Q¨§/*¤<?SÇ}9]
?ïƺߏr#?z•ô‹~ã?Z¦1Ê«Ê?W(€Ä?uþ¦½OG?wzØL«?ï"óJË?íI".}?|Æ#K?qMàQœ§?"pµ=dzI?Ö"×KÉ?íÈ«Ä®4?"Û ßF?p!•=̹·?`ܓ°Ë¶4?°¸ˆˆíRh?"§GwÐÖyAGN3FGL J0316.1-2611@ku‹y¢ƒÀLá@&`½À9™šMÀÀ;Ší~óûæ?¿^&"¸@'k£<"?ýµu_Óz;¿æ4©: >¿ÔS"™Tq¿¿ÓLw¿vš^¿æüv.õ$ÉAGNbll?ïò$ò8þ?T$¢j8Y?@–ƒŠ9ì?;d5ôû­•?S–tÀ®Ú?PS¯Ôãw¤?ïNµŽÜk?',_M{/?s0ÓÇdÆ?yê¼´0û?'cò˜jC?ŽÖÔ?îïT¿º?‰é
VV_?ˆ"Hu#hq?w-—5»Í?•Ó¹ý¾‹?'–!85°Ï?íÅY>ÆËg?žAʵ!]¾?vBj9X^?rќŸ›V×?°q4*Â?x¢Ü–÷Ü?ïú°§Ê:?:þ6zÞ?,º‰BzI?#‡LŒW(^?<3âmŽqõ?5\9rI?ïÄÔÂ~Y?utf› É?_eR¥Ig0?[Vdáºb?u¼Jâ?q¹'Â?Á*yž?uvY=}øË?zE¦ÂÝ?oŒ\[8?€x¼ŸA?jDhÍN˜?ïQ̶|~V?~|¥©'#?lfœû‡ß?["<O8?'9•´B?|§±—ÞAGN3FGL J0316.2-6436@q˜Œ€AÀG` SÇþÀ9™m~ˆœÀ;Ƨ‰Fe?¿àáÕ#[W@)f],+@»ˆß¸ö¿æ¼ö‹ÝÕ¿äèåËæ¿Ømÿ!ˆ»Ñ¿Þ÷YñÁsAGNbll?ïíZ•'û?`Ú«~Ëå?3aOã6]I?1?Z®VOý?`9@±ª–D?_YLË¸?ï"%@MÅR?…
fë¨w[?e|:Ó+†Ð?eÁŒE~Õj?‰—¡@Ù·?'zg™Øá?îõ$´Œ±v?‹êÖFIð¢?"2RçœDŽ?r ËöcÎ?—B?þc@ï?‡p»»Ì?ï7‰ìIâ?ˆ}xhÖßô?@m•yþ§á?<Òè"<…Ú?˜‹UÍÖ¦Ú?ˆ;}ON+c?ïù™~86 ?JëCõõÛ,?'ˆ‹¼ð?*ŸæJ ?C·âïËÂÈ?E2Le*+?ïײÒáÊò?oë-QD/Î?R-³ñ7?P|1sÔYÒ?o@–»ö=B?j`i™ñ)?ïD¡ï?{ƒÇþ
wG?tHʘ˜ÔT?dä%U8du?Ê˜˜$h?xÀV–?ïØÓ¸›´É?byõ-¤?.o'0gÂ?"\KøEò?r¢ªÇaÑs?bЇ>AGN3FGL J0316.6+4119@bÅ}q?À+xÃß¾AÀ9š÷È3áÀ;1‡ëlm¿þ?0Õ4û4@
Acôq+'?þlËð¦¿æb;qE< ?ïéå}Ya¿âÂÝÌ4² ¿äTæ–nä1AGNrdg?ÑÙ?ç?§ƒ¨€îü?sыØû¬!?ƒQp½,ÈÂ?¢<ág '?£·àÁIÐ?îԎÓu'?«,YÇ~&?'™#0}ù?ŠÄÄ8Ö@?œ!"þ™r?§VHB+L?줒/øt?¢Vã\HdÐ?Ÿ¼œ$¤ª8?‹‰L'ïu?²ìHßCÖ?ž1ª±"Ä?í¥õÊ
êY?²û)
úÆY?"jÝbÏ·?¨B̜:¼?«k¡m0V ?­®€Àá…a?ï'ÒrJ— ?"—³'ŒH?a\R©z?hou²nÝ?‡ELo­'?'£(`1É?ï¦æ»­¸?'P†¼›?fPgÒDV?kø	َo?€²7/w(	?ŒÇŸ"
 j?îØ(—g©÷?Œ	æ;ff?‰='n9+‹?vh³¬ f?˜\+Ú6]X?†ßnÊiïS?ïBFü5<š?"rU3ÃcÞ?GÙ¥ûãé?WînÿXb‡?–øSG׃U?"-RՂ+~AGN3FGL J0318.7+2134@dZ{ 1ίÀ=¦B 6mÀ9CYLVÀ;FüÎX%¿ò%¶Ëƒ¡‹@ZaðàÓ??ýeŒ¿@)¿È†ÙI»h¿âÒÔ
³È¿ÚêYùN=®¿Å­åMn•+AGNbcu?ïü©õ:ë?6z²»	?q›ÿzö?·à'qY?8"!ßé4?6%jUtB5?ï•S5©|ˆ?Š¡ä-öå"?gξÙâçn?|UƒÖhöÇ?"·'ç>?J¬>"gº?ïA¹¿	‰?ƒúbÃTå?˜9ÔÙ?t@¶ã†>Ÿ?Ž‰ŽvµDï?eڀ殙?ï¼ÈF;‰Õ?v4r¢}>æÅvUjL>ñ¶xW4ö?€È=Ÿ¾?v0zŽ@?ïþ4ñ×>? QZׅd[?	tޗÿI?)<néôK?&SºÓƗ"?¼_øŸlò?ïÛ:,6?mp
=Áb©?Rï®+%x?Q ¹´oEw?kMüÛ-ó¹?fåÞU<H?ï›PÎØ?x£œtæÁö?t¼"ú·b?gcQQÅ?}½ÔèZ?tkor#=?ïñ€©?M4´ÈDɎ>փOõ	½>џ5á9Ï?\®\&¢þ1?M.xë®TAGN3FGL J0319.8+4130@bґ"DžÀ*ƒ þ}IÀ6VdöúÀÀ:C,x.?úw°:ÅÏ@»ªõâoÌ?ÿŠ\º³¿Þza+OJ¿â%^>#Ò¿áXïYXz¯¿äĶ köAGNRDG?îOÿœ­Ë?³ÇuH?Y
Šió00?c·TÿW'?®r«µy>È?²È¿•åV?ï\'Þº5?•šŒÏ)õý?töºDQ™?zëäÏ~×?Ž`++*dÓ?'¡Oהã
?çiÖÖ2t?´ÿë™QÜ?¦À(ûQ
œ?›7,}f§?Ì«Úf	ìŠ?³nÌC«t?î	7X©1?§%ÿ,Á51?`/tDEY?l€y0œ@Å?­uGþçê?¦è-}÷ª?ïÎfTó¢?¤×å݈?KXF0Ù%Ú?Qê9"«.&?ž«qW»V?¤­pß7ÉË?ï¼̈́ò\?|ß	äÒ÷b?bJ}b8|Ç?`/Zâ'ë•?xÌZ¨—_??w{76Ï}?èþp>ñ?³‰i{{?¤¨Ðw´éí?™ü¾ÄÅ?Æۊ!Mú×?±Np‰"Ž¤?ï\|Æ=U?Ša¡hl'S?`Q}ÔG½?^!pWY?'nµ²']c?‰Œyd^¾AGN3FGL J0319.8+1847@d¢ß?–À?¬",2À9a6€Å=À;+£»[‹A¿ëq†œ€˜†@W¨ï¢æ?ù&:è¸?î¿^·ñH'?ÐG¢Ó¡t§¿Ñã%•L:¿È›ÀCì-AGNbll?ïý;7
³G?0Ò#ÄJ8
?
ù´¾±¢?§â,$cf?2å)˗S²?/÷×!?>:?†ŽÇÁe´'?cÈÉ'¾ÅT?d†ÂPÃÏ?†žL\?ƒ³~
Ò^?î´""ÂÐ}?˜Üj°•7?‡µãá˜44?€Á$®¦=6? ½}¹5?•û©î¡>ò?ïQV«®3?‰ª^|¦Þj?("zÏá¡?,gäIf¯?•¤ïv
—_?‰•'8æí?ïþMºëEU?!A8N ''?2æ¨æDä?¾½Îv@˜?%š»òì)?ýŽàÝ?ïÚcu' £?kh¥²ãáÌ?R—D¨B(??PÙd('J?lPçÜÅ(Ä?fs®	Õw.?ï[°`8, ?‰wKitˆŸ?}¤9¡/'È?v.Z_2È?ŠAË/?…¬E«¡R!?ïÍ9…C¡?i·e•"¯?`Z#zÐ?	ákì8~?y&|»òDæ?hçê"øˆ¡AGN3FGL J0322.0+2335@dCsÿ¬*À;—ý_;ϺÀ9P»Ú6BÀ;F>{?æ°5­Úñ@$Š
ÛPH?ÿ"«€÷·1¿àtŽì'Â"¿àUšéоŸ¿ßçÃô*¿× cڒUAGNbll?ïÛzRg½?hÏ­UžÌ?Rd"ŠÐëK?OÞþù…W?k¿CŠ‹å?d ŒÓ½ Ã?ï\/eô%¬?"'6ê¬?r¼t÷¹š?qa—1ýـ?•ëûkd¶?'=‰‡Ú}°?î;¢Û=Ä?"ò›^,ëw?"ÃQz¦LK?'-֕·?¢d)•²?s(;"rí?íÂr3À?™."·Z*á?hJ;óÙ#›?f±¢.¨†à?¶‡šÿ?b?˜ó3«ãz?ïó›ñÁ+Œ?NU¯:Í?<þaò33?2«‡»rGË?QÂ\î"ãÃ?GèTÚy;?ニRêކ?}6‡¯ÃóÑ?`8ʧè?ZA¥õ"Â?x qhÃÒ?z.}
K…?ïP4l²õz?'-¥ð· ?'ê"Ñ»K?uÛõ±Šã‡?‰P^«ø?và(ö¤ä?ï2&è?yz݁#û¹?Z?:'Ő?G‹C¨Š>?˜§v\?y¦c҂AGN3FGL J0323.6-0109@fþßÞøH|ÀFœäÿÉy[À9tJLTliÀ;i'Q¦»Á¿Á7ð㓞ê@
¼¤ªnÓó?ý¡¾ Œ'u¿äv%7êI'¿Ú'e»4Ž¿ÑíÖ/ª›'¿ÐñèŠÃgôAGNbll?ïk"Û¢'³?‹Q•f1¡Þ?VqœÊ,?R͝ôôfu?'4ŠÀ´M?Š¿é}?ïg•Xl~?ëÕˆ¼ì?nžä~'¢Í?€†œ§lV?ŽrðιÕÝ?ˆ'ò ë—?íÁ)á$ó?š†š÷-A®?•» ÐP­?'«²1~DÚ?©'…ˆq|?–3
"֊4?ítÆâ?Ÿí¨÷ýÊ?ZH´úžV?^ËÞÛ++?³öÕXˆÜ?ŸÔéÊáž?ïÌM ò©U?sùköý³?E׃ösN??uz¯?w?A~?rÞÿԇéZ?ïÑ7‡©
?rïy­?U>÷}d*?R'-×æÁ?r˜Òðƒ?nVÙ:Å
?ï2FÈ!¨'?Ä
ÀÜò?"Prã:5%?qzªO¦.É?Û•XQ?y©¼ØN?ïNR*ð¬?zå'E
g?P¢{›þâí?A¡ûµ'öy?•+'à)çS?z=™öÜAGN3FGL J0325.2+3410@czªŸ{ZêÀ2±Þ_œGÊÀ8ª_!ΆáÀ;r‰EŽŠ?öÖÒµ'@º³PÏÑ9@¤Íˆ´o¿åÖ2¼•Çþ¿ëÕf7I¿ëp§
ׅŸ¿å)y<¤AGNnlsy1?ïö-cÿÑ?O1>gދû?=n±äõÝw?=3,cÉp§?H"+›éá?H£ù´eú?ï1íL?¢•!snìÛ?zÀxýTŒ?|§e•Ì?—‰½èà'? iQ'r™L?îxÅøáí_?•ð\'('?"ð´Í@~å?ŒµA'æ«™?œöŒ©?.?BMʑÈ?î3™ÐK1'?¤›IvQ?‹"r?O?†¦Î†Aj\?¥á?Ÿ¢ÿ?£_ae?ïûz4ë?8´Çýð?)/Ìï?!E'	Å?7®
I2±«?3)Pvª?s?ïŸkêxž?Š)IÈ@¹?i®Ôë/ˆŒ?hÖ¦˜m8?¹P6*á¹?…õœe¨q?ï@÷þ ?xsÛÏ1?‹¢Xz­€?€þ¢¼¾ÆÕ?'p×pa3?‡`db¸Ù?ïú'×?'PÈÚû¿Ï?z­+aJ¥B?kø+oÏV¤?}C×o6õX?~Ýà>àAGN3FGL J0325.2-5634@pí ßÞøHÀHîà_PÈÀ9ø¦wÎm·À;øñ¼p^7¿ó¼lzQªÃ@í«B¹c@¹´ß›0ž¿ãu'ªMW2¿ÝÊÉTÊÚ¿åxþ(º^`¿àX ŽAGNbll?î]Þkõ`Y?­-O9;D?bScgRÿ?cM	xšµ"?¨üèG?¬ßʽi\¯?ïYåa÷Ÿg?'1Aúýl?píY¿?}ú5Ièž;?ÃOÆGê©?ÞÀh†?íû"V*ü?¡úì­®G¨?ž–gàäܹ?‹Ù‡_7g?®õח,â?›"¬Ñ>R?î䃯êX?•ÓFŸð¢?_1þsn§Ê?díHq­k? ¾?ƒÄÄ?•T)
0?ï¢w.	ӓ?:Nc?L$U{q¹?RHg<m ?…Ÿï*7Ÿ?ŽÇ4Bß?ïÑõV¿æq?qƪÃëV@?To{¢0–Ÿ?S5cíðÈÒ?qéuÃß9ø?nZÁ10?ï
ˆ³å—–?"꽧®™?‰Í.oÊ«?wYÏ*PZ¾?'ÇíÌõÝ?zßTVËì?ïÏ*"?nÔ-Ë¥?,«L±?'ˀg½]?w…"‹\#ö?nˆ)P!¨·AGN3FGL J0325.5+2223@dub¯È°À<I¥ÒÀ8hpeÓÀ;Rs×Ûõ?õWéÞ«qˆ@BFBÚp#@¡êöÙe·¿ä¯ñuVKð¿é1-o#ú0¿èæ¨ãZû¿ïÿ?"éøñAGNfsrq?ïé¥Ô#@?^<uú÷Ž2?Rbû%mc?Rx³'–«?ZQ\&¼V?S¦V›ÞÐ?îÒðlÜD?žæšŽ×?…•½Å\Ü?†,eÚ<†u?š×êŽÅ#?™V¿[HpÊ?íï³Çö¬Î?™±Pn*Ì?£·@™YJ"?'RèB9¯{?š›ǘš?Ž'΀?îC뱋d?£%L|ƪ=?m:["§ø?eÔ¶Ÿ:£?£Š²WøÜÃ?¡<«£yšµ?ïó(Åà¹-?Pý°¤æ?N#)Åéèö?Jr *Êæ?E9½ÑñÜ,?=FÑȚ¾I?ïw|ßà¶ö?‰Œò%Ó¢u?w¤K;²E?sJáy¸Z?†NÃÝdõx?'ßõ
ŽÙ?î"`µ!Ši?'@ø͐-?íþ!×4?ŠïÁ›¾}?ÖqH?£M¤"ù^?ï…nóífå?'á­nâ†?}âíÁwå?ra{r͊?e™ˆ•|?{µ©œ¨aAGN3FGL J0325.6-1648@iÀÊ`ÀJy¢@1HwÀ8þ­-]À;.InÞÚì¿Ý4gX\@ØOØŽZ?üì¿[u?¼â¯ã ܿޙ`æÂ
οÚìýf?¿É÷7ô&óAGNbll?ïôãBô¶?PÒã½)@Á?,-à'Ö?'6Æ°µ*?R·à÷¼?O>·
ð?_ýŽ?Ž·j€u‡÷?fNÑu'Ö?€'üþ€¿|?"Š§} ÖÔ?ƒönããÁ½?ïnû>?‰¬—<è?"dzxvF?v€?uA9?"TëìW?…ovq ?îñoC"º?œH–‹‹þ•?6n\2âÌÓ?;*×EŠB?¯ÄOgÈñ?œ<©LÁ®ô?ïù¥Œ'Qd?B*²-H×?*q'
zïË?'Ïå"-?BÍoU4Êa?=ŠÌÍWyÕ?ïÝó.û?jÆÉÿ8å?Pý>ît¾?P©•TÇõ?iŽ1Ä»¶Æ?dä¯Òù6?ï‰Õ0@"?}ž¿JŒ ?wï1v#¯?jIy5a?ü<YS)²?yÆĕ[Êi?ïvb»i«ž?x
áƒM?'¬˜,l"g?$td™Ð?'O]è]?wþí®á(ËAGN3FGL J0326.0-1842@iý^ß)ÀJÉ?Àà0À:P3:~À;ê'Ô©:!?̐õ_ß'@"KtG¥†@¤ìԍ¿ç­üÉÙl1¿ë¨ËÓJß?Îq€Ö()¿å)Rü{;AGNbcu?ïٕ"á¯ï?q­R+™}i?ÝE}þH?"º(B/­?rÍ2Š+;'?qŠûõ¶{?ïsï!Ð#2?YŽŽ9n?o|*?¾	Ò?}±I;mÌ?‹%,û¯ºø?‡t¿?|‰í?îJÎFŽHœ?'Q‡êÂ?‹LÏ/‹Z}?xœ	oB=Ÿ?¤çÌðm˜?Š}AÖ+t?îâ"`
m?Ÿö=<²Ö?V"™#OTð?i%š'i®Ø?¡,Å7°…?ž§¿ŒÈP?ïñ‹Ë¥°S?Yñ¹©U§?ÆÅg/Ń?
ÜJg2V?[›üÓ)M ?Y"$Í-\'?ïË·÷±/–?w&ӖÑüT?]•ÛR?`.£?rã0ÃTœ?p¨8ô‹S@?ïUp´6í—?yq‰ë0Ò?{iK7?jô'Ø¿?ŒïKUR'«?uѳDp1?ïǪÙ)sä?ué‡
¨?W?Gõ'Uû?SÖ¤tí©?vZÁyªäa?rP§Þ»í˜AGN3FGL J0326.2+0225@f—ðŸ¥LUÀE7´_î}!À9^9£¼¡À;sK@p2˜¿Â2õö¼µ@Pß:šˆ?ÿøaՈ]¿å>êUÁ¿ß‹ß¼éá¿Ù¨ÀdDß¿áà¼:OÔAGNbll?ïòÁí1'?Nx eäª÷?69Ï©?R4?/so9õ"?Tí±e"º?J¥Þ5÷÷'?ïiLxT‹?‰M1';‰ë?l»Ê€Ë!;?kAé…pfø?Ž}ïo*»?…ÿ"ҖO?ï³ÆãÌ?'­`FvçÕ?…U"'Yö?t1ô"wϕ?'€ÜR^™)?xld&Ð	Q?î$'̾¤?'ÿ	h'?^`êæ½2¬?Uá"»ßô+?¬ÃÛÙÒf6?'£›S—¨?ïú3B¼W?7¹sÍVÞR?&—¹CëÙ?$=Å&>?Bk×ë#¸?4•Ç4d*?ïÑ=«˜Zæ?qs%ûµî?UQØu±ŒÇ?Q'ßd­ÀI?r´0ƒ1w?mÆyþG
ô?ïšTE§?oœ'#Ü8?vaÚUŠN?eI*_ã?|"{Œè*&?bâ}¬´Ä?ÃxBå?p–²ÑOq?R"šfJ›/?>Luq.w?T{Ì6÷N?nÇ#¬ã¼hAGN3FGL J0331.3-6155@qO{`(^ÄÀG)´Ÿ¯]PÀ9¢ó_2•À;Ãþ+êi–?ßʆ˜ØJý@JêßÝK@œÁ€hp,¿Ûh€{¿áýý–æü¿ÙS	÷>0¿çè0ˤٔAGNbcu?ïò™ $£#?R{ ̺?II-ïÍ´?H[‰¥cø?LPRæhŠ¿?B¢IBûè?îðÚ°æl?–XÚ×¥¹?~Àìœ.u
?y¼J0>Mü?š4n½:/?'ë†N;E?ï*lÁ…'?'æÖZ·}ý?'´ýd¥Š(?r'ØV¯r?'Wé q?zB''Á>c?íȐ ?¾Š9m?†Ôœ6óUN?}«b^¹Ý©?­ÈïäÓŽ?š¯^ç?ïù¯°ÿ‰/?;P*04Ôv?3‡ÈIE<š?.¹ÿ1'Ÿ?>ú®häy²?1€#¥K.Q?¬M•#?9«óé?l:'åP?edlJ™?'vŸßê?|!w~N«?ï¦ëW¸‰Û?nº,¼"›?r^öX4?af¯¥ïó?zvõ#[æb?f'Ýò¨?ï_ôÝÀ˜•?~ú^°ÛnÂ?|[
r§bë?c÷Dª*?‰ÕAÎGq?z++Z[AGN3FGL J0332.0+6308@a~] Y§;@Ø4¤À9Aq
.W+À;E}ö¥ä+?ډWw`3Ç@
~ºÆ@¥àŸgŽÚ¿ä@Ë·€¿âbƒp'o¿çü5ïêÍØ¿áx¸É	É­AGNbcu?ﶙÝjÄ?|3'pñ}†?sðî=Øw)?u@ºÃÕi?p"3Õ¿@?jh}\Ë?íM¶äz‹?»ÓĞç•?‹ÀõdVÒÜ?'íä•-ˆ«?´Usš™ƒP?¸ŸxCZ3,?î"Èãä‡?–†‹¹ äÖ?—¬U ̾?‡·8›ˆ?¡ýGC)ƒ.?t»j"?ì³à%U`@?›bµ½ø¯»?²ñ¨{/?…7x7*Uí?¶j ¢k]?š[ó…n‹?ïâK ×h?~´BrWi«?\ÀªÎÕd?j‡I»­ç?^¨ǕzÛ?rxõ
vsÄ?ïæàãõ?£—X^¬W?u¿Õ"°Ê?{2TšBØ3?–öS4ٜ+? WbËþÐé?ï_lT<]?ö
Ñ5z~?Júy/?rk$ð\o?‡" -d?vÒ<°Wõ?ïŒãcù5?~ªé²êƒ+?zY"ÑÖ?búdíåÖ?–èM/(y«?{Î"<NAGN3FGL J0333.4+7853@`Pz WŽ\@2{Ä¿¸TÀ9Ç~è=k›À;Ìëô°@¥¿à— ïèõf@%Ê>ýí@"Äÿ£ä¡¿Û•Dí'6›¿èñ%Ž¿Ôº˜ñí²d¿â_†«ßAGNbcu?ïö[òô?LKSgL!I?1LÛó'?,gØê¹»?Mívž,í¸?JOÉ$eÅ?ïqx']?"¥ÜÅ~©ó?v"çÂKO?p ?ˆWç¼u
_?'€]À×?ì?‡Ì¯'÷‹_?"[ÀF1â®?r´ÝeHö"?•.«nk3#?'™É¤«é?ïß^RyR?‹›Ú¶š?X£2SøI?Sä‡;Žš?œát¥]?ŠÿٗõûP?ïû'wÐàÇ?=üíØmøç?#õ·ŸÛ?%QûÅàÏ?9y¸y•Ú~?:Þu÷qч?ïÒñÁ›8?t¾m%Tȹ?`¤«cx!Þ?V¹Œ­:ÉÊ?mHb˜ô&²?qcg!-}?ï"_a(S?t&&¼¡–F?vH9hûÞ?iÅòáƒ?«–Ç"Dè?l'"þ\h?ïÓ'Ø"?d"[´¦¤;?Dx=E9?4"àæ0ª?sÚe‰ëµ?cww$‹ëAGN3FGL J0333.4+4003@c3›Ÿ˜·À)óš?±Æ·À:ã'ñ·À;"b£cF÷?î…pƒ[û»@q¡Šÿ¢ã@æ¿ßÿY'?ïý°´,0Ï¿Ç$ۛ`‡ï¿çþÏ$¯¦¿ïÿ	ø&mAGNbcu?ÙiÄÉaø?Ìúóf>£T?âFu?r0Ê?Î1ª;9ð? J…¿…*? 7ÒQ·{Ù?ÃȪÀÕÀ?ÄÕË)š¿E?ãÅ
¢nÄ?Æå	¢ž®Š?Í#µo/…?ÀæSuaŲ?àõs¸<$§?¶wƒîÅA©?Õ*-¥Rœ?´5'à§E?ÁÕ×ꉪ?§njñÚ['?ÇCAô<Ø?·ÊÈA¡?æm…-j¶?Â币?¾
R°ÉXp?´3oˆá"?Ýhi§?ÍQ[ÎnÑ?àŽ3롪?Íç´(T÷˜?œóÿ^Žd?šªtp/áò?Ô'‹©?È[ý'ù?à6¨
ÿ'?Ŏ-ñ'
•?Ç
"°â"?¹‡œ¼n?æ	¬wÓÝI?°|ØäJQ?Í9]y'ÍÐ?«áyW@?µ?áR9	–?Ÿpê)Ó-Ò?à0Ýô΄Ä?··"Nj?ÙÓ>NwåÈ?¸{¹Žö`?·, ö=?¨nՐ^À&MIXED3FGL J0333.6+2916@dªKÀ5…šr¦çÀ8ÉðeXImÀ;=¨;i?ï-@ÓÃ6 #?ý¶É™"{¿ÏgÆ°_¿Ú¦¸f
{¿ÕNÇ,ò|¿Ú‹Ù"׬‹AGNbll?ÉÙ)?ŠcE:?î?|6³+ú!t?}{š•?€»t'Ì¥?~¹ö×rk?îF:'ÃûS?±4—ãì6?ñ±Iâi?›ÖìÅÂj¿?£#1ʎ•?«abp†¼?í"$yµù? æuRÀ×?¦-ë¨]–Y?–qù|	9/?§¯Ó
?"˜"CÀà`?ç0"°¡s?¯§55ó? $§bÜ£l?šÄ²ÉÃÙ?Ï6‡Ú%—?¯ug<þw»?ïwcR?¥¾Ý\þ7ó?€'6žV¨'?"tOncq%?"ôËnÕØ?šuL[˜ð?ïNhبðq? a%ÌÒ²é?z®7m +?"¥µPÃ?®…57?™ìVׇxË?î«%X˜â?"1[ïIac?—wœÂä"?ŠW–
ÖÃ?"ˆƒ¶r1:?"Tœ«š­?켍ÿ v?™Ý~L–n‡? M	'«Y?ˆ×
ó|œ°?·˜‹E¦¥?–(màÂÈÉAGN3FGL J0333.9+6538@aUDupÅ@p4 ½À9SFS¡hÀ;YÜ&Ü㛿ë…hßÜ@•ÒóW{?ÿ-! a¿ágZ™t
¿ã;©MZ•'¿ãEMVlj¯¿Ã3{}¸AGNbll?ïg7v†;?‰§~Ð
Ë¥?c̚ç'8?\ïÛ-Wbþ?Ÿ}Ñjö?ˆŒØïYt?í«ò`žë?½ˆED"éè?'=i2t´?Ž5¸—¸ML?°X¿Ö¤yã?»"ÏIB­é?íÕݳ‹‰?˜hy0Ó?—Mònuh2?ƒÖ1iøHÔ?¦û+Ã]?'valgÃo?î¯MrFü?"áØÞºV?AG¶÷Ó´?EC«'ê=?¤Æ\b_#?"Íù°Mü?ïÜKËÊ2?iÚótj—?L€¸hŒ©?CøvHÿÁñ?l͆]3+5?g'Ô
Gä?ïS®0ˆ?'&˜Ÿñ?dë¶n?boiecx?‡¥ÙÂ`"?"ù¿î×?ï=KÊr™?~y~ãâ?"QÑþí¶?q؄¼–ân?Œ¤?Ûéô?tôôΑz"?ﶬ[WŠ?p‹'k
8¶?#zmòï?ÀÀi–ž?'ÿy¯?pv—½ÔóAGN3FGL J0334.2+3915@cG_ét£À+Æ 
aƒÀ:3æ/tbÀ; Öwpyæ¿ñ[µ
8h&@	'C¼˜L=@èØÞ\—¿ëž"('D¿áî‰~ª'¿Ñ§ˆUà˜¿â®+VÅßsAGNrdg?ïî.Ã{¯?`!äó«z?5Í
|eø?4c‰fb¯?^`ÆA'õ‹?]½AyP·?î~B	(?±òÀ``q?‰ãsD½¤?—'¥uô8?¡¥—?¬€aÝg:&?îYÿfcG‰?ŽõVø—þO?'
€ÅWûy?}»$Ù©)/?¡ÙI8×W­?ˆÉ~²º1?ìrü眱Ò?«£QH/	Q?iD•°Ô½=?k–äi;ÏÚ?»ôû…ƒ?«v6lgv ?ïöx¶äÇÚ?I'¤êü± ?(=÷Ûæê‰?"aå¢Ú~?PÓ=&aÄ?G¶òÁ.{d?ï"Ϥ‡M+?•ÝôH°ù?p].&'ŠÊ?…:hùÂû?'Ã1Õÿ?‹ïYÙT…?ïB7ÝUË?-.0Å?"R™dÉbõ?y,déÆÿ?‹
˜'SFp?rëâfe?ï­ø\ƒË?ˆ?ÜÑâV?T2*j?Iƒž,Ȋ!?œoa*Ë?‡§‹þ.!YAGN3FGL J0334.3-4008@n˜ºà;>šÀK{Ÿ³À7ã$Õ¢^dÀ;ÁÀ)P[?÷	ÿºùf@
PIC•×@΁,æ=¿Ü¤SÃႿãoç‰ðõ¿ãT!šsx¿ä2Ó:éϬAGNbll?ïö՞Fkc?Kà^€ùª*?0þ­%ž)?0§YîŸ?Lž†<e?HjýÑR?ï˜a›P}ò?‹Sw–ýl"?fŠÊÕkùÄ?|sƒ»¤ñè?"D懥?'o Ê$üº?îÓ@%MÜ?'>¬Ъ[?Œez0²JL?ƒ¤|/~-e?—e>CÁ|?‹ÈË^@[?ïgúM—8?
Y•ì"?K8g9"S?RR½|θÚ?'&ö$d,]?ŽñÓu+?ïûùW'®¶?5À8ʸԪ?)Uv,†z?*Ì8S냴?3Š'n"	?(ÃJ<Íå%?ïÛûU˜°2?jüØëÞ?RpäQ]ð?Qf˜€‹öÚ?jÌ8i\FÉ?duՍoM˜?ïS<Hì¿?…4{'ŽWu?"öᜈN}?~¦×wý
ñ?†:(GëÔ?zÓ|TtÙ?ïÜñ.ù4+?mÄÞê¥0—?G{î¤?G'Œqeù	?m+ŠúÇÀI?kYí‰<H•AGN3FGL J0334.3-3726@n¶â—ÀK.Æ 
aƒÀ83A!…À;é/"Ê?òd>0<]Ô@@WŸÏÍ?ÿD@v½¢¿Ù?…¨Ö'¿ÞÐY©êt¨¿à
ƒsVS¿áÍróéAGNbll?ïûÇ´èˆ?6J®ä,Ú?¡ʤl2?‹?º£(ž?9ÚPÞ'?2×HËåDš?ïdQÛßG?ÇΓß6?qHËèú•?zêJ´ °`?Ž*äꁼÏ?‹†/
`Û?E3¡ÿ?"÷Ááˆc?¾â	'(v?ƒ¢ârm\,?šnæS
Ýâ?3Ïk–è?ëøê¾`‰"?§5©Îþ§Ò?…]ÏÚltR?MUÅm«ª?½Œð¬|\?¦#c†‡úþ?ïý²~©"?'£ ±£j?KŽxÚr¦?"âY" ?)²Qzx/ð?#ýÐbۊn?ïÀÜSH?}æ·ƒª9?`k(¹Mç.?as­ª‹?w\BYH•?wܳIkøW?ïU ³©»%?ê7a°?ƒÇ˕óýR?tBžÝ9¥=?†ðs?yl8ò»K?â_[/?‰Ã2Ý1zË?'Q$Å8,7?lÄ{ǃ5?¢28§àZþ?ˆ³"CÜ)µAGN3FGL J0335.3-4459@o–``þG™ÀJs^ŸÈ‡ÄÀ9Èi*–¬À;ŸÈå·^¿ÿ€˜N?þô@ÅC–'¹?ýL ?µ?DkYÀ;¿ä3JJZ¿Û¹69y¿ÁíõçMWAGNbll?ïñRNñ ?^A;([ÿ?'ݔJék3?)8~ýŸ‹Ž?Z_¯œ÷W?\upHS2,?ïžF+×ô?‡r@¸w˜L?b;
™±òu?g픊‰È?ƒß±ÉðR?'Þ7Ì~­?îèêfÝüí?ŠS#6½‹¤?…Q7&ɳ?pÀKq±àÆ?˜:—»ô?‡{ÛN·÷?ïoŠÇ™²?‹ÃHÈ#>úÈ ‡H?Y½¿Ìw?'&ä)?‹‹}QXp?ïùi&Îå›?J£¾{¥‡?!‹"¹°·?Œm¯qê¼?FB~'¯8?Hö=^>è?ïß4×*ÒD?lxT&.?Oþ©ž±?P)¼žÅãP?i	i'î?f·¢Ûm¼?ùwó?uF©?wÒdāK?`P[i]"»?ƒ‡Ð&ܑ?rã:ô.ýÐ?ïå胦W?b/b9¢5d>Ïô "¬>Ѻ(˜?jº†æ'?b-Úõ¬‡AGN3FGL J0336.5+3210@cã@¢‡À2ß?@‡¯ŒÀ8¥ÎÆ¢aÀ;£êUt?ð"éŒùM@†GqD@ÿ•!¿éÅÉjý
¿é—£‰â¿ï50ZÞj¿ïöZNÍdðAGNfsrq?ïíûÿ
?lÕr‰ôƒË?P•
¹i'=?Z Q [x¢?UJúÏ
t«?fQoýʌ?ì0~(¯`?½·2á–]?¦"ØÖЙ¦?§­U¹õùz?³1¢Uf*?¶ïŒLK}?í*'¶é'?¡>Pëܱ?¨h˜''Ò?–.‡ad.?¤ïÑê¼?—´b¡˜þ?å™›¿[?¶=³Â#v?ì&¤""4?³»É·ßùÒ?Çírì~r?²l×ôO?ïÍäûJl=?­&ÊÈzRŽ?P³4"7,K?mÒe&2{?tàµOêb?­ËŒ?îYd_Í?­‰‡h>­»?"ËqÓ¸ìt?"oÝsé%? ‰0Ñë*í?¦‹ sÝ°:?î(6†é'?–ꟼ5ŠW? ~K7zS?Ž—cMFµ?™ü˜­»ƒ‡?ŽÊEz¥¼?ëãq«¢?¢%;r?®ÞhÙòÊï?"ÍjAíT:?±uCk=$t?žøIÔêAGN3FGL J0336.9-3622@mÉõÀv}5ÀJó²ŸúÜ«À:XSy#ØLÀ;ç@Çplz?ãoú¯@Á@«"ªO@}¾€ƒÈø¿ã¡EßL$¿äM՝Î)¿í2išV
¬¿ïÿ¬vÒ*–AGNfsrq?폯¯ýÖ|?·ÌÖÐå=å?Ÿ–Gywv? º‡Í!*?§9Ä\eÜ~?µXŽ€"n?á‰õ#zzè?ɨ"µ¸£?Ð$EQ_?Ä&¦Òxo?ɟâçsõ¤?¼¹Ôž8 í?ê!£üóA?¨¢<D7?¶í£i`£?žQÛÿjÞ?¸CôÿúT?¡nVsÛî?ØÅQ­5œ‰?º??Æi†V?ÜÄò6Øs
?Á7K./Eñ?Äëx5¾W?³ÕõOÙÏB?îûÕ×k?Â%Emâ‰?ª8»AæÓ?¥×úeÿ?§K&F )T?ÀZüŒZa?ê4§«€!?¼W¨LS¯?»!Çv²Êÿ?µÚ¾ £ÉÕ?³=SJ§Y{?¦±üď¦!?íüN®?›np­N?ª©Q¿Ý?'í(¤°W?¤‹–*1('?áJ2S9c?è:>–™?«êÃ$Ná1?ƾÁíÜÎ?ªN £®X?°°‹0ßÁ¨?š=^ŸAMIXED3FGL J0336.9-1304@i+eà.©aÀHr¶?¯À9÷×fƒÂ˜À;Ͳ¿-?¾ÔT1Qÿ@
I—è¥#@\ 2e¿çœX¸uIP¿è
LTþp¿ì,í4‡'Q¿Û Kb\ŸAGNfsrq?ï'¡|ßF?ÁLz§Çø?u¾Jý?wø¿ýÛl?–Ì<Akt?›vz4îW?îß©ü=RÇ?¬PaÐ×'×?'¢´ÏÅÆ?˜´(ÿj¾?šÉïJKJ?¢øÊB?ìIΧå¯?¥—ÒìŒàÃ?¡ÍáÑ3?Œ¡Iƅ{y?´ËOÞ?¢.î¢Vú?ìDà†àPÛ?­W8z^¯¨?"á!U€´?—uÆ·§$?¸ ³ty3$?ªråy箘?ï¿ø2M§u?#Z³ŒØ?VWf¨x?Wây(€<Ô?zn
J¨‡)?~*o"»Æ?艹Ë"£?##È;€z?iŸ¢ë"ˆv?~5	¤(?~`ß°S–<?ƒ.L¸x(œ?îÀø#iì?‹\ˆ/þ+?æø
<?v¢ý×?ò%?™Yˆ"Y?†fñڨå?ïKÔÖ
R?†ÁZ£›˜?sÚpÏ¢÷[?iI1§ïE?'ŽáuI"ä?ƒÏÁpcšAGN3FGL J0338.1-2443@k\_x5œÀJNVßà¥ÈÀ:Ç×-xßÀ;Çå–È.?qê™*üµ@µ
a½_G?ô"=!±í?çÚ«»ÁGð?îàÃdCK"?Þ²~àä9"¿¼y¤Ëj¼AGNbll?ïœ
¡ˆj6?žo´¯#ãm?Cdýè¿8?lf-NtY¨?‡ÇÇç¹!?žAø1¥Jš?h*¥Š?K€VÞ{N?k/"Ô¦:ˆ?|ª÷2ьn?ˆFþJë?"Suíùù?íðđrŒB?™AÕ¥rò?žâ]o×/P?"rúTŒ¢¥?¡'ˆ/3Ö9?i½óeôÄ?ïf!~ø%
?•–PR‹Î?QºÑì×K?ebÉÁ(?' "ÿG«?•
lhԗ×?ï¬ÞVT?½8ËL‰¤?9»/dáW?QŒƒÃã°?žÃwqM5˜?½;²ˆ¨Û?ïÙeÓT·y?mÈqf©;%?SâáœG¶?QÙõ
uÓ+?m»\Ö{g?g½£³Ô¦\?îB>
t?¡,N"Þã?¢HH:£·L?œN*öÇɸ?˜‡'ÌÙª.?«'¶°Ž?ïØ_9m×@?pUF]¦\?GßôÈè«?B€¥lž8÷?pì§>c	/?n¨Ò¡ÁéìAGN3FGL J0338.5+1303@e±ú€Ïž8À@uç_ö	ÝÀ9R&"©x4À;+_ùdÛL?ãyc)?@M<yØÞÿ?û'Àä6K?ÿ
¿ÀpÎ^È7g¿×ë´Š¥z¿Ü
{ÐA1µAGNbcu?ïíòRS›?`%c$/9Ê?K¨žtÒMó?VJ9\3'?VG'k|?RÑÙsp²?ï¤ñ:í?¦œ*¤?x¨tøØH?Â1¾íÿ¶?™§7»"îQ?£â,ÛUP¿?î¢1KÛ(?"sBñ+?K/½ØŸ0?€tž]²?œFEg?icƒÎzN?éµR¸)/?¯ BuÞbþ?'º4ÝÙð?Œ§'SzÚ?ÆÓt""ØG?¯ð´åMÃ?ï÷¼Cßö?C,#WD É?:":~Š3"?3ìÊð̈?CÌÒ©³¼C?8ÏÝ[ðƒ?ï£çeK֐?ŒšmÕ³‹?k±|÷äŠ?xEë|ÿDÅ?€ÇiÈ?…ûBDâÌØ?ïi	4mV+?€ŠZ&?ÕyÖȨ?pEv"çK¬?…Òõ€?z‰qpÂ9?헂ŏ
F?•{·Š?ˆÊ~—hÅ?t0ø;'­Ë?°*š¦µ8?"‰k+ЛíAGN3FGL J0339.2-1738@j\¿ôw6ÀI"l?Ä;.À9µè«î0À;Âóá?âEz°AÉ@§¤d"ê;?þÙeÿä&[¿³ó€çWMÖ¿åù25Ý1Ÿ¿ÑÞh_S¼Y¿áɱD00ŸAGNbcu?ïõÅ3GÍk?H"ßEpݙ?1²‹Ï|•]?, Ö97È?Pöƒ«š?EÖO{=?ïPmëNª?Üü:¯?p…?j8#?n§9ˆîl?'Ðò´-'·?ŽÀÕQú ?ïnÆԇ¤?…5Øyà3
?…Z'¿;ß?s¡Á¼9Šó?'¥¶×–?<0ÇmôB?ì¥8;ZÉû?¢¼…ô–?z'+I|ý?xşŠ¶2?¹3Ëv,úV?¡ñ¢ $-t?ïú0§VŠj?9 ½›ìÒ>?*A|ý^?#—dô¹?@¬ý¾'éi?49+®å	?ïÂÃ.Æðr?vꎺԍó?_€aÃ7K?Zû¡Ù|†*?v¾P+À8ò?sDÔ0Éj?ï'Þ.žùÖ?qsçª00?x¬¥Ç?gã†Äø'?~òÜøß:f?e)Rá°©?ïæ(h?ƒ-‡«&%?xtzA¡?d~øBe»?˜ß÷HŒ¼?/"o{ñAGN3FGL J0339.5-0146@g€À
¡©ÀE9…¿ÈŒÀ7êûgPÀ;Ao¸õs?ø
ÃÁ
w@1sHL@«,Tò œ¿âBü÷Àt¿æ=ä²F¹£¿æË°ŒÇ›'¿îB"¼díAGNfsrq?ï̃mL"‡?sˆøP ^?p¬Ÿ\†{ ?pTSò?b#SâQµ?^–Ëà÷é?ïy›ý¢È?ŒÜ¬é­ƒ0?löQ¤7*W?v+é͗'¨?Š[l-ël?†[›îCÑ?í ê麼?žŽºÒÖ$…?§{ímH†@?–¾"µ5*?‡Éïj	?'(E|2–Û?ﬠKÜÄ´?"Ö¼"-i§?Ur=)?5=?`yH÷=?')¥kŽQ?"!¨ÚÉÌ}?ï×ü?În…?i^ïù€]?n_ÿyY{?f›0©—\?SGª#Ð?I§'r?ïʛSÐY?s]Hˆ?Œ*?\+ƒïìÀ?Y¤C§+ËÞ?s§u2…°þ?mq­à*$$?íÓGlÑ?Gª":œ:?¥Z»É€xG?"ځƒ\È+?šé¿"ŒW—?'»€Æ¥E"?ïíp—}ñ¯?i³àÅ
·B?CC™6sÉQ?CÙ9¤ntç?[}[±
?hny\nµ$AGN3FGL J0340.3+4130@c9 _ñØÀ&;¹ÿkÀ8‡"õÎNÀ;YnÉw-@shÁ_†@qÁ:Gz?úAÔ£ÿÏ¿Ð$ð¿ßî¿Ïéx¬0—o¿â"‰ü²\x¿ê;õ2,ßPSRPSR?¦§p'øoý?«¥(¨q¡ù?íȺü7@?²ÜåœÉ?™™À%·"?‰¡÷-•Ý?•ªÈ¢
	?¯ó]h
?é&uá%?Á‡¹¡ÌÄ?ȲiºžÄ?¿ø­ïD¤}?ÅàœDf-Ô?³]>î?æ LëYï?¹4–òù›Þ?ÁÒâ‡ìjn?«"ø—ª?·Ié¤žÛ?£Êï=˜š?éó9*•l?°w`©uö ?¹´Ä"ÛI?§±¤=¼˜?¢VCÍ?©ËifÊ/&?în¬qIœ?®25Wãî?‹ä§g–æ?•s3@ƒ¯¡?¥ˆ!Šô?°ñ°1x­m?èÿ‰_\(l?Á1T¥‡?Ƽ8{­±?¼B³jr¶?Îì÷$9EF?±rG7‹É?ã;Ðúó•}?³ö	òr"Ý?Ä#ÄïødÅ?«µ/½šÆ?Åý}Ld+?¦oø‰´·<?èÂ};'?ª?ÍâE?«è"ÿ‰;?•F¯BUJPSR3FGL J0340.5-2119@j¹ fèlÀI—Ï¿ÆT
À9¨¹t*tHÀ;ƺ_ÿ¿Ó"(h@!͌Fµ@½j?¹ÔM¿æîNm)Þ¿Ø22ä{7¿ç§›ãõi¿çuê	k)AGNbll?ïê9Èß¾}?cƨ}-™i?Y®
õ¯»?`³ÅãÑ*'?QÞ`/W÷?Qå‹úèq?ïYY—ÃM?'«k[Ì7.?p_,ªêº?~(\JBÁ3?½ã
úû?º©ÍY?îÚô‹é¾Ü?ŒK
D›s?øîÌÐ?'X)—h
ô?"!uE]ž?|è·ý›k?îé1Ü4ã{?'óä"ZÇ?t&ñ6n"?rÍpw¡œ?ÐC{Š!ó?¡¥N%j?ïók,HÞ@?]àâr?Q?P¡¶;ðTê?Z%·Þè-?AáÅ8v?;78év§g?ïÍþÿ¶`?q§N^?úå?Wµüް̈́?U`¢ÎgÔÀ?sà;Ï?mê>m¾k?ïâÚüV?}0ªCí4?€ŽL­,ql?x• ì:L–?~ñù˜

	?kçNîы?ïÇc¡—Á?qØ&7U¤?Nې¡j[k?Eví#ÿæ¯?xr½oá1,?qv¶€?UAGN3FGL J0342.2+3857@cu¨ÙºÀ)¡ÃA2Ð7À9c2:å¯À;sƒY¼3ø¿í$GÎÜؚ@8rP)Ž@ôR?gôÜ¿äSõCŸ£/¿é%©K­¿ß6Á¡å1¿á	pe)
ÌAGNfsrq?ïû¾°æx?9MÕÅÂÙ-?	a–²rÀ˜?ôǙM?>ÞD¨Æ·"?8Uq*²L?ïzµü"S?Œ%Ýêi[\?p^4ï?s4qq"]n?‰Iô±;x†?‡-œÂÚ4Þ?ï".ÎI¥?…<=È1?»cÉI$?gšü[2é%?•Nv5ïÚ?'ýœºj?ïÇ4¿Ð:?pe&•T[?æöWù¿?á¢e°'?|=f8&`µ?pQy}Æœ?ïþ94?)¦ðŽìQ?€Á‰¿
?ŸåTâ?) NÓE¡?&ßðÏ?ïՂ³¤Û?r"T¾Uå?V¿Œ™•5±?X.ÓØ"Ï	?o†DÈq÷?l<ã²­Áä?‰hI?i`»L¶Ù?p"S¨´?R`g#Á"?~ñT8?e‰wNŸW?ïôùPÎ?Fá6ŠÀôE>ñÛÛÚM¨>ç÷"b(†?UɤD¡+?FÉ6œQh0AGN3FGL J0342.6-3006@l|¡A(¿ÀJCr_˜ìËÀ:Ûk3TÁ"À<?'æFñ¿æmŸÐÀLa@ދÞðæ²?ý‡_úfŽ?ïÿd"$©>¿ç¡jé?¥d'qya¿ãÈï˲ùðAGNbcu?ï̇÷)ö?…×J´lZ?ð=ݶŸÿ?$S»oßs?y<pœ4m?…ÊÖí%÷z?ï'Ï(O]?‡ÕÕy‰?gfÅmy?hOœÞè;?‰r±bè?"<7ÆBRŒ?îfª³¿¬ö?÷Ý:»å4?ŽÝâEpQÁ?OSy '?¡ÝÜ6¸*?Œx¤@6‡ï?îëæ
÷ œ?—|F'\?B4…"Yq÷?KüKV? øͳ—T?—H…z´ÄF?ïñøý¤¨?axË"'£ô?N/ÛÉT?Ç|RWô?\s+f H‡?al®Cê¤p?ïÖt4Ád?kú2q3¢?U#–Ã0'Þ?R ¸tC?okÀ&Nú?eOp"{ž?îëTÝÛp‡?"×/X0Ž?‡+Ï!÷Ý®?†& ˆ=4?–ÿ|¬¶ÈM?Ê^@Nºþ?ïËÆÙÝpM?l>Iàsp¯?4›ð݀¢î?*ß'0—ÈQ?xÒÓîEj³?kî4}S¤AGN3FGL J0343.2-2534@k"$?åÉÀIÓ½ÿªo«À9dïS	'À;Áozân?õIu"¼gÐ@ÝŽ<_@z®YÒY¿à«îz
vë¿æ™,¡É"Ý¿î\+~LÐØ¿ï夦Î;AGNfsrq?ïШË!P?|Vóvìÿ?aËóÈáô
?fS-²ìU?m‹AJKËT?v5-
é?ïphú¯"?ŒJ&Špk?nµ€ÉC¡?v*ndËÕV?Œ8}?³Ù"?‡p^yí]º?ìùÞùӞ¬?£¢m9Փå?«&U5XÕÄ?™Žˆ(	Ú?¥;»0ô~?™¼:¿Ãk?ïVŒ´âRù?'«B ¤?;@'úN?ÕôÍ×?ŠÑ5$?ž}?ŽšzõQ–Å?ïߊá?{赈zôÑ?cÿÅ
Ì8?pÙxMŒÚR?[Çô¢‰W?j5ë¥z*m?ï̉r§^Ì?sìñ6a܁?\Lg·÷4?Z'/úXž?rº³…T€?nd•"Á¥?î™Öšá?™Ø;&,ö"?£ÇbÜlr²?'̆¹"¢?—}ÿsãÞ~?Ž˜n.-{>?ïØ»ú±P^?uË®Ü±?cèÿÏ(Õ¶?b‡Ïå¬|Ö?c[bª?q¼7®¸ÿ¬AGN3FGL J0343.3-6443@qsb¯È°ÀEԛ æÀ9fÖ 2¥oÀ;´UhaQ¿ÖYÛ¬AD¡@ÌÝÚçÐ@;}ßÔ¼Z¿Î² yL¿æh»j—¿Ül3,۳οåÿ3¶AGNbcu?ïöD%&ˆ³?OS´Äy? ÞËE÷Ú?ƒJ©‰!¨?Q[õ:{v?MBYáY·?ïkb±ru¶?¾Zoí`²?l»°yÀÅ\?s›ððCM ?øg…JW<?ˆp+«ZB?ï$ Ç°ü?ƒÆ'æa?"K¥lÎñÓ?uM[Å`g?'F+¶Ñ³?~;iµ?ï	Úó'D¢?ú<qèÁ?QoœNaƒD?Oác-è˂?­§ÁÆ ›?·m‰ø?ïü¡gÝùŠ?6bè†?Î$ׇ˜Ñ?$Zð?»è?5Á7©ðæ?3…]Q&÷Ó?ïВ€ºib?p÷n/ŒKZ?Wv]n?SË#ìéÀ?qò"G§×?k\´W©=à?ï›USøc?s6J—6h¡?vD53õm-?fn¶tLTV?| ë†A?kŠ¸Hõ"?ïÍ ˆåÜ?k?|Í'à?8"-ƒ'?-¿Ÿe?w­˜šç/£?j¤ô8bAGN3FGL J0343.3+3622@c°ƒÀ~à±À-fLÿyÀ9Õáƒ=6ÂÀ;x?ǖ,'ÀXî$`\Œ@ßE	¬§@i0`¿çWœ=Q³ì¿çޔiÂ7¿áÌøàÀ¹]¿ÝyHª­óAGNbcu?îûOað""?°â¸ºçµ?o3º§ž?w2FX'×ý?œ¯¯äj"?¯öP KFr?ï/9
+¦? d8Äڟz?xp0
<À,?‡ô벒¥?"lÝG%?š
ù$è‡?ì5XÊFŠ©?¦Nx`žWB?¡ŽÇ&ÇIh?šëÚ­+?µÖ°8?¡ðÜÔ/VU?îƒE+¥—¡?›­A)0Ÿ?2;ÍQøS…?9áŜíÝD?§§5«¶ç-?›}@·DD?ïgß9®D?·Î堖(š?qą(éñ/?–|/Ÿš\?\¢Fàf?²q§Š "p?ïÉk)#?xº\	¦©ñ?[¥ç<†	l?a@R\lˆ?ta˜>de?rgC£žKI?îàï€Î>?ˆ£kèKý[?‹| øN?}Žî.ï9?–W
)ŸÈ?€LýE–â?ï«Z¢@Æ?s¥s–Ìqõ?
ž«çG­?î	Éh¡ç?…7Ý:Mò?s›£5Ùé†AGN3FGL J0345.1-2353@kEi_ªŠƒÀIm|_Ìï1À9Bn
Ÿ–3À;ªªùš‹?æé»áJ»Ä@{Ú\S=@CU_'òc¿âýږ‡Ì¿æë)ʏí¿æ2ًn€¿åš\Y""BAGNbll?ïÆ`¿ˆkŸ?tG¢'F?j¹4ù3Ä?fi†ÔâoG?o‡6<•n?iÅÒò%­×?îJ\B~³B?«OGUfS?‹M¾U¹æƒ?'«ß)aFn?¤†Ì@D?¥.ܞgcÛ?øhBE?"î>ó?'®ë¹—¨ã?'«y²ÊËF?<@?Fx?‰t?;+¢?ê¢eKþ?¬ÑêRu—?¦†ÈÐv¢	?–'̈A^?¿©qAÐsº?©··®*ëÔ?ïìŠÃÏx?\Á,©Uø?P~
À딤?In†uS?VljϾ,?SÒÀøõG?ï{Eû¯/Ð?"'+?u
Õo£q?zÅ"=¦&?†©:¢F?‡uÇ%š£˜?ïwš®õÿÕ?"bÙ#ªM?~tdüçñ8?sUÙÝøµ[?'ß!¸µ\N?s		›ä'[?îˆà")î?¦üd²4°?'ÁOÒ6T?v¦âËóN8?œ"¥"®?Š/CìPšAGN3FGL J0348.6-2748@l1~þáÀIr¬¿ç<À:ëWÒNíÀ;ÒþÈÈ[N¿œ@2 îÊê@ƒg5™?@6Ÿú0Þ¿æxxi?¬
¿ã›åGO¿ã¹Ý³h¼q¿ïÿÛå:úAGNfsrq?ï†nKbª?µÚv1Ø?ržÿ¦;-?tæ9ºG?…ýJëw?‹À¢ô–?í»R£³E_?¨=%Us%Ç?•<{Ó£$?'lüß?©¬˜>™¦?¢¤À 8|?ëúð|‡î?¦ª‡½ùö&?²×w™Á<? $°*Ù<?ª¢	n;û?—mTÇL;?ìsJFír?¥¼@³Z}(?¢–×`c<ò?—Æã"]¡c?¶@ùþéy?¡w4X»ò¤?ïÜb#‹ ]?q83ç"åc?Y›}L™z'?Vè')"õ?fЯÖVj?k'ïÁ!}"?ïM§³bÃo?Xk^ÅH¤?߄^ê?yj²õ¹ì¨?	£ig|Û?"š]'ÊÇ¥?îA"ºÒ‹?"<_6.UÍ?¡<¤~­ ?ŒÉ"Ö]¼–?•T3¦#)v?ƒ°Š,
j?îõX<8?ˆñ{.÷?…bUXέ‹?xÖèy"¶?–£Íؙg?"m˺ôø+AGN3FGL J0348.7-1606@iè¾ß¤?æÀGË <¶jÀ9wÅüÀ;Ä	Ñ:×?çt[5}2@ڗ.u0@»#à)¿àx7YáÀ¿ç'fÈHr¿è2ee4¿åH6¿H™'AGNbll?ïò»ø-?RÉL¥£$Ì?O~Ùø Ã?LòžÇˆ!?H"5'æ–o?@¤ó}ˬ.?îï¡E`?œÆI€¥D?}—"߸8?~Ú†'\?šËq|âí?˜'ÕÁBI	?îÔäÉ)?ˆágî¹¢?Ž66°±²A?€+ې^l?–ah©né?'dW««?ìàäH‹×\?¦–))?šº¦ýsB?•pÆåͽ?²J4;!èS?£ôiõŽ?ïì'è×^?—"°oI?^áçó»f?—–Q†G'Á?@4$í'àØ?4ìdZºîÖ?ïªmqÈ?'SE¡›­Ý?f~Ð]ڊ}?bì€a.W"?‰ß>ÚÍ?~ž"
g>w?:e4@?vaÎ	au?}Ýò-?rU¹Û"{Ê?€Bâɨq?gÒãÿy¶e?ï4þWzx?‡¾ÀEsà?…iá†ri?n^^eü2?®Nœ¯?ƒÏï=þNãAGN3FGL J0349.2-1158@i<c>ÿPÀFÞ-ÿ틉À:.¶(E™gÀ;¤¬§"W`¿Ó7‹¼%#•@Qð/¨d8?ûÀ
ÿ±¿äW̍ÀP¿Ã1®õ\Ÿ$?¼~=Ù»ƒà¿Ø䢃šv0AGNbll?ïî;wOlÐ?b³rãQË?;Ï»X†"?²ÇÒÓ?¨?`òª"ø?btÎÿš?zZR÷?†\qEù0?eÁii•Î?g{ÂJ:"?ˆëƒþÓ?'òÍ~Ù½â?ïiÐ~25?…21ƒð4è?ƒ«3ÊÝ´Q?oÜe0…S?",	îø8?€ñ‹{§Hâ?ïOˆ$7~?"]xAÄ?6HZ¬Û²?Ca~t5?•µÚ–ùá?›Þ&î*?ïø|)µõµ?Mø¹—¸?AÿÎYò­?b¯
…V?LØoo?Lh.gâÏË?ïÖö7îó'?m@RT€?T'c9À&?RïüŠ|0­?nÁ3"ÃP?fïå›Є?ï‹…BA?rÅ"´??v ö€]‡?bi¥x†Œ¿?îc^ÂØ«?ksQ£7/?ïلÈà?c'Ɇêêî?3hĽ¤}?(AœóŽw?r›UêÄ?bv9˜¸AGN3FGL J0349.9-2102@jÌ¡ á÷×ÀHƒ-••À8ÅQa£ÊÀ;Ÿ>øcSŒ?û¨:üÖ)î@í-(­Z@Þé	nh¾¿àzZá;Þl¿èù›âÊ¿ëòPË°©<¿ïù¤ë¡#AGNfsrq?ï´àïy
?|ߤ3‡1.?yGšÑA
?yGôÒϗ?hÜÐ$Ãø?f3供¾?ïm,'<û?ê®ÚÕkZ?n4îè·)D?sÄX¹vß?'Â^+PÞ?‡ªå'Œrü?ì²u:Àú?¤úx)"g?²×BAz?¡Äê¤OàP?žTV÷ç
n?"'éò?×͆Ü?ŽÑ¸Ö­?rk9q²?{1ՒԐ‰?†$}nÝÜ©?Š?kp×8?ïÖ)r?7£?mç$ƒÄM~?o†½Æ_û\?jBt§D¤?TŸ 
òp?QIìÒ`"s?ïƦŽäM·?tå"ÊA¼•?^ßÿýÚ?[Ý
k2?tô¸¡¹"?oüš4gi?ì÷üó
Ì?¤y&¤²æí?²T¨ÍäÛÕ?¡Ê
F7èg?—­¾i²¡(?'º8wJ!R?ïá•Vò]´?rçô£±ò•?^Æ5»òµ?bUøofäì?^IU:?mй¤Ò‹ìAGN3FGL J0351.1+0128@g[@îÙÀCÍÿÒ³—À:qbBë7À;‡»DLÊ¿r4G9b
@
›mrÊ!ø@r*ßý ¿â®õ惿éì¸
Ú
¿îùW'8&b?éM°&±AGNssrq?ïnHÁÈ?'þš£z†?`
w΅l?s88¤¸æÏ?ˆ!æ§
è´?ZW¿x‰%?ï‡kg4Ë?"ÌÀíл?f¾]®fò1?wËDö‰?ˆuŽÏ—Ì?÷;)Y'.?ìgæpâÁ+?¢ùP5
;? ‹÷š-?‹'a)÷±c?´zÐøøÇ? Lz…kà?ïü¸f¨? ·ì-ú´ô?CdÐñ?ZëÅÑ%
?ž§ì挀?  ¸ß¾?ïá»—<â?u€ÆÅf?A7=]Ëcž?LFñ"èSX?i÷(ãEŒ?sO1œRW ?ï×)6¸¬?u-Á*žˆ?T÷"÷si"?_Çx¢B¨y?nxó·&?lŸ¶àšÂ?î¬ÏZµr?×D[4ë*?¹k,?yø~¦~?›Ü·ìäñç?‹4v¡"\?ïÝü–OHy?sC\v҈?ÖZM.á?9VxÞqp?pƒ­›B‰è?rô5¼»_ÐAGN3FGL J0352.9+5655@b9ø -à@½¾`Mr¥À9¿aY·+{À;j¥.ùÏ?è
~A4¹×@
ßôA…ÜM?ýT@ÿ¤n?é_{Ò£[?ïú¼3Cñ"¿â2	6¬Üº¿Ù£}`Ül[AGNbcu?î³b4vÔ?´"^bµ!¢?'ÏûZõ´?•ú¾ý ? Ý䁇E?³Ñ"kÑ6?ßQ#]ïÊ?Ö8p¦Ó‹O?Ã'æ};Ùº?ÿt+˜V›?×é©#Y?Ѽ‡!iS£?ì#ccky?£¹þÐ_Z?¢(šÌ7n?ŽÞK:Á?µÐ—€¼]Q? ¸­§€?á»è—"ÂÖ?Ȭc±ãV?ÖöL5kOb?Ê2´×§`?¶GŠp@`Â?±ÀZÓªk?ïbäŒd°a?µ¤ª¼'F?o" =¢ç?!DšÏÿ¦?aÔËÇþ?³-glJÖé?å¡Ñ¢ýú?Ô#à£/?¸'h¦:D?½ŽbÑ'ò°?Íl
7?Íñ(È\`å?ýÃ?'­2!"?'ðœ¹ë?™hµŒ?E̒ë)¯?u«ã$%?ë'NŠXÞ?®gWuY^Æ?¹E­o¡i?§\öšäbå?¥O¼óaS?ÉÙ*BAGN3FGL J0353.0-3622@mÄô@¯¹ÀIUøØþ3À:w™Á݅'À;®0Ô´!Û?¶aš
¸	@Ì<C¨ p?øÚu!??Ü¿ïÿVëQж?ïýÍ«øty¿ÐGЬ³ÛB¿Ê'H/wDŽAGNbll?ïèœÄúÎñ?sâ æ9c?ÑOTð? ²çê?fd²îê'å?rìMÜÜÙB?ÌwM¦?ˆ­z:ó_Í?f#@Œæ‹?jèî2!Œ)?ˆ
ü´ü3ˆ?"UÕBfÕÁ?îû÷–¾·¥?ˆüO‹EÂ?…G¦387?yš{ÿCY?•Ý:½@?"8½=½¾?åó(?†+ßa6í ?YÆù¸??]¼T+Þ?‰Æ~µ(?…Ñ,#K>?ïó)ÑÆÂÙ?_ĆÎoà?­'ð=º,?a'÷×ra?XQƒ`¶8ã?_lÙ³jD$?ïÛ¢ûÃw?kË.ŽŸÕ?QEñSš÷?P…[Ë ¾?kºˆV²?f"–cŸXÁ?ïtZ nÌ?'_Fҙ`?xîÎ
ñX"?qlñäÂ?†rë?¨?€mòX?ïàÍð¹; ?`™ô÷NÅ?JâÚK?=pWm íé?h°VhÒ/m?^ÿ*ì2…ÉAGN3FGL J0353.0-6831@q¬' ÄeÀDcX R…ßÀ:;Äõgö‰À;­…¨K
E?°QÔ
°g@
èlXï
?ùÑ°Ÿ¶5¿ã?^…zˆ¿Ýå‰ïNú0¿àì7¶(¢?¢¨´"œ¯¤AGNbll?ïÑKÝ#12?rÑ'›i™G?9HV¡* è?4Ã;fr'?uŌô@3?rMWsô·T?ï…B%$¸Ø?†`Ë ;š?gŒTº©øú?i¨}F®Ži?ˆÌa…¥¹?ƒ9É~|p^?î'¢ßŠâ?'%ã$¹.?SºÇy—??~Tê1qp? "¼¡?‹aÒ7W˒?ïv˜Á5?'«JfÄ?F戁	¨?Rý Òb€Û?Yø«="?']W?Áõ?ïð"¬—?X$ã"2Jô?&|Šž`Ê?µ_˜n%
?\óSÞÊ1Y?WÜÿ›fX?ï×Uxœ7È?ly£÷ŸÁ?S7…'¥ƒc?P½Sxœ»?oÄ»qµÄ?g`Kԛ¡|?ï[¬"¼C?}ôèþ*Y?€ôÇèäfç?v®¼á³;ê?ˆ 5'õªv?rˆ6¶óŒ?ïÑp³`.?l-õ£‡~?6]á†û"c?5Øs^yM?véz³÷}?kYoÆ))AGN3FGL J0354.1+4643@cGŸfb5À«
–ìÀ9·ß(ë²À;Y
W—Õ¿'ÙK•'"f@iÆ@ì"M@
ä?Z2ü¿â'¸…¼Ì¿çÏNK+f¿â¶ë±`Ø¿æSZ¨m
AGNbcu?ïT"×jµ€?'ˆ€Žþ?kŸâ¤ú?e¡Îájä³?'û"³=
¡?äÎìϱ
?ê
ÞÊü5?ijѺ&ú?ž"Û…ˆL?ªj	N¬b?Ãö	b%?ÂWeþ?í€zÏ)†?œvDР‰%?™R¸>h"?…Y0tœG?«NöïFZ"?•äê˜D¡?ëù.Åî¿Ä?šñ7}}?"lývW?uHÝâo[Ž?½¦\0é"?™¼þÊTK?ïݍßHœÉ?lÊBz?3Œ?NǤVhà4?I£,À»ø ?jÀ7³`˜.?i;p±Õc?îC\v"œ?¬öLÅLó?†cüZ­@X?"øË®>Â3?¦19'ßl,?¨ö†諌?ïB?'^‰E?£ÂEÁ÷?r"ë	ÆÏ?jÈtH7?ý‡ulÎ?z<>h©3V?îÉ☜o?€CÏ8f¿?uꃕAl?\IÄU1¨? ¤¡:c-?}í®ùšfAGN3FGL J0354.6+8011@`Lþ?5Ÿõ@4¥_ yˆÀ9†mpEã9À;ٞÞ|øy¿âùͶט@Ld×pä@ü?_'`¿åÝë«_>Õ¿ä>ñ5'g¿äN­i"¿é ä´AGNbll?ïúõãŽ}?E›×¾?4}gY
ž?B<t-ÿ+å?3ÙéŸÒ'?0Q¹…9_?ïº8B/œ?ƒû¨5siV?hmð›Øg?jÎ	¶S¸á?v­Xñb?€qÂOÇCÆ?ïHîŸ
)'?'7›áìj?ø$Û[x?w@éIó"©?‹ÌMZà?yŠå~KîÂ?ïù Ô1¬1?P€·ÐÝAÖ>ö@ë Ã>ÿrí4©fÈ?HʨFþ=?Peø£±rÄ?ïý½|fœ±?.û€ó]	?%{OcÊw;?%¸¦Œá?YÛF;?Ií"l?ïäášÓð?iӗŽžá$?Tø‰ÄÝe±?Rç·ƒ|?`¢ †Q^?e628+Öv?ï¬í6Ô?q»{.{?q驟ɥû?fvEÂó?wŸÔ,xÀ?i¡ù€µ?ïÿïÖg*?'W]ʌ†Ü>Ôô""ÕÐ>Õ:÷§cf?wR2®ÿ?';"y—nAGN3FGL J0356.3-6948@q¿÷À*ýÛÀCéUÿæՍÀ:C|»<'À;ßÀãŠ~tÀlÌìW@U<µ'ôd@<šà–ƒ:¿èúJÉÒÇc¿×Ù­w"œ¿ïÿ׶µ´,?ï÷7ã=ŸAGNbcu?ïÞaG¡1ò?€!û2$è/?V'ó+–Õ?ZÓÉ°S•Œ?fU>¥GÔ?}Òºç5óq?XUñ=?ˆ!;Wå‡?eL咿«i?r̈́Ö	¢?…G°"'5Ñ?‹Âõ•9T?íd]¿›-e?œÕ4#Ú6?¡ª/VïJÝ?ª	d"äŠ?¨ô¬Ê)Ù?•itÆ|§?ïñ0ž(R?f§û#"Í>ÆP¦ë¯âo>ç¼çד¯L?]"RB‰?f¨yؽS?ïó©yE?[ž™×V¼n?A•i"i¼?I<¡©Øh?Qø^6É@?SÀäÉZ1é?ïÙˆg~P?q‰œµNŸ)?Q'4ÅÓã?Q´åL
õ›?n ]AöVË?niä†!?îÚºˆýj$?‹Å/)©g?¥tÑàž@?À)wÞãð?":rO?"d±JÌ?ïþ¿×­Í?0V1çÂÈ>kǑÿlXM>| Ø¯ÄHQ?$Éb¹Ðr?04ýåmAGN3FGL J0357.1+2325@ehß½jYÀ6ppCßÀ9ü³1ñÔÀ;˜Ûmy€¿ß>^Κ@
¦•°ÖÍ@JÀŒ}¿äÆî–Ì	Ù¿ì—Õ°\¿Í™Sƒ_Æd¿Þ='7äYAGNbcu?ï[D0¹~?˜­ÿ6U?C"_j"d?BL
Ö?"ûLÚ&¼'?˜YÔeP|?ï^z#)P?'ôÆÒ<i?rèW´ž5?|¬èïØÁ~?ŽíKXª!b?ÿzïÁa?íH*4˨y?UèG…-Z?"÷«µµ_ò?èÓ~šÍ?°€Ãj뉻?™ò…F"?îHv?•iœÓj2¿?Eu5g™âµ?KÖËåz•?¦¹f«• Œ?•>üÁ¼`_?ïÜ'Û*ø?uÐgg<'?06æ<žÝÅ?0•« ?ó?púÐ>'ù!?uCè/ÿJ?ï͵'zÔ?s'Šøg={?YHÜQý»?S{0M©ÄÉ?s+îIŒúo?p«@²æf?ï')«÷?µ¦0|Ø?³¹ 
?m"ÍŸz˜?'Žî>
a$?xü'^Âo?ï³qþ0XI?nÆU°OÚY?>–q›?0_°ô³­?'/¶‰b—?nÊ÷psŠAGN3FGL J0357.1-4957@p+i€,
JÀHb`GhtÀ:+à¤&À;ù)CÆ(nÀE¦}X@V†´åzn@DŽ*GQ¿Ý!Œ@hâ¿åwºXáA¿Ù¤ZŽ}¿à¬$vAGNbll?ïûÅgõÿî?4T":6bh?yàË?Aè³Gú—?>TQWœi×?3la«¹*?ïŽy¡v]?ŠôïI²"=?gÏd*Áó?|tFb2Ï´?†mßą²Z?aêîgD?ï'ï}{Ö»?™Ý-ºoÊ?Hÿ‹ƒ‡?hó8 ?'zëËÃ÷â?{Ÿ4#
V?ïÆÝC´Ø?vS°'æÓþ>õ˒lܝ?5
[9?|{'x>"?vKRÛbpq?ïýxË1°ì?&^Zç.k?807Œ–è>ýám×yv%?12 \"gÖ?$+ÊIìÞg?ïÝoo#¤J?paÀ
·?Næc½©>?N4•wg?j×ÆÛçµ?lgkΈ?ïà?q5+¨ö¿?sÒ:<¥l?`몡ì[Ù?éæYù¯?kóvA
?ï÷+âuÅC?LÜc2Xï>Êź[Mp>ՄìQ?QšØmÏ?KüäPÀ.ïAGN3FGL J0357.9+3206@dX6m
JÀ/ù£~õ©eÀ7q=Y&ãÀ;="Ö¼@üFØ
@ñˆ\…g@"Bè\ö¿ÒJÿ5]c¿ã(vÛmhR¿ì§nœJW¿ïj?©¹!tPSRPSR?hå|$€–?{ʎ'?ï×ð1ßSÁ?ƒ\ÛV?^T¤	›r?j/L_ÞC¹?zA2•u'ê?±–·=`·?î)í%v à?¶ pûÐ?ªV:£?ª~†>"0b?¤jÂy^Q?—‹·ÅòÜ?ì(³OD®'?¥µà™ºÃ?´…Gዹ? '@¤š[?Fquœ7ü??GÒ+	ÔòY?ï´öh–[:?€mc7_K@?[N)¢œ?µDBîÈ?f(¿Õ@'?rþáœèƒ?ïÓÜ<›*­?‰dès,®›?eû®r%Ú®?Kt5)Ø?dZ'-'¢?vÄ]ˋÑÔ?î#hŸ§?©x–í&en?­˜&šüù™?©¯ùU¸?¯ðôNé? s)Ü1ª?ë˜"
úr*?¨¼|Ù«"¨?³µw—3;?¢ˆõ‰8á?^Ó@ëÀËg?R~CT£þE?ï¶
{â'?séB6ûч?}EñÃPž?qæe8ƒ8PSR3FGL J0358.7+0633@fê}æOUÀ@Çk 	ŠÃÀ9EçbzH›À;s® 9[k?Ütëüà2R@ØJl4܁@É •¿ãþÚ®ŒÅÌ¿é9Y¤e£¿ãu5ÀØß¿ïÿqtâUAGNbcu?ïû#à|ˆ?;(¶ èDÿ?EÐWࣧ?0Á'['x??‰]·æ?8¼ï©#â?ïXÃ]Þ?–ùÔlÔ>±?ŽÑÓ›?'Ó€6´,?–ÑCÛË8?'¦­|›?îÕD¿Á?‰ûN"¬‡Â?"[ŽR/ü?PY;`L?ûîõ×ã?}ä'!ûÿö?íÈýT ‹?#/»?ˆU(‰q?Õ\M8?­ZãxÑF0?šwùÐΆ?ïý. q1?(Û«¡èYï?íÝÀUýÀ?u$N‡)?/'m&Ub?"@E•ÛŸ?ï•ñ-q?ƒ1¨Ëd²?pâ—ÜJ"?i8m‰5=c?'K±LK?~x±\J?ï?Txʎ{?~‹ù^*7? ý›ÂV?vK,A""?ƒ
ÊÅÔÚ?lYm%½"Ï?ïf2Í:c‡?}$y¢Ôcï?uümÅD‰?aÄ. >
?‹uÃÆÔ?z÷ÐÌUÂvAGN3FGL J0358.8+6002@bàP7P@è‡@%´ðÀ9…З]À;Nâ~ú?Ý3ÑÏÒ!@)ðÐq@$ˆÿÃo+¿ãØÑÂ؃¿è²‰"p	¿ã‹·	RJa¿îXQúøÄAGNfsrq?ïߝöå=÷?c§Fc8Iù?Y;£$Hèß?SoæÍÐ?cÄ7u_Å?^¹xž'¥¢?íª'4¼'?¶å.<Ÿ?°Èl»I(?"'5E]âq?°x­K¡?à?µrˈ˜Ú?í`=½O?Ÿ%˜±`at?¤…z¸3áÐ?"Š–æD?¥v­M®ô?"½‹åq¡g?ïgÖß}Ý?ˆÒR<r?]"ÓØÁäó?]AX[?'DéCÖ
?‡v]Þ'v?ïìÐᐃ?VòÌǶà?VÄñç"x;?Oµþ*1'?O2—þlUÚ?Hµë.H"ß?ï[+µ:‰ê?œ¹C0•ïÍ?koÇJnC™?pvç¾AÐú?',u¼AP?™OÑñÇ$?î¢s¨6?'—ÿõõä>?™cÜúÕ>?‡€g§*½?'MÀ/ãûñ?"#ÒÒ§?ïÙ}e9a?h@ªr`kå?OVÀF'~P?BPt¬Ž4ª?n¬ê¦öÓ?gM[4O"AGN3FGL J0359.3-2612@kØädIVÀH!'	±À:"QN"¹À;Û4̐fë?Ó½I¬ÇHÔ@
Y9Ìö@Œ4ÿf'&¿è‡-á7¿é£¤"ƒç¿Ó‰J†áÛþ¿æHðLÙ¢AGNbll?ïÎÕÇXÚ?vœµ¤ÝZ'?-¬PpOÝ?'ÿL`ÆBñ?w¬ÖâÎ4?vN'<ÛP'?ï
Ùs?›'Î!Ìމ?z9ÃþlŒ?'€Æg?˜`¢S½Ç?"¶Þº:Aþ?î!Qc' ?'ú3"ÿe?'ªÅ³Jg$?|Öû=
Rª?¥à h?‹,߀/o—?퍏u(v?¤Tt1¼L?*ijd¾??¿2g~?´öFXSÿ?¢‡W@¼ZO?ïï¯Î—Û²?Y0'§?"»ɏx?œWW)¨­?^IK3ƒ?XTüî
?ï¶â¿Dª?'G"ÆôÝ?bæ"Ï#vú?fë'öíP´?{V{;™?{©õÃSÊ?ïM²\€?v>0‡õ;Þ?€(A·?g%!ˆ?ŒsÑ¢¹AÄ?oþC®÷?ï?ŽZ÷'?'x~8	œº?zgM}G?kNì×Ä–?'‹ZÅ&õ?~À˜í'a6AGN3FGL J0401.4+2109@emÌÀ7"À7UH¿ŒrjÀ9˖‹È¿À;‹³ß•ý-?îjÌÌÒJ@á㇤N©@ω REr¿â½¨ë¿áŽ"Ç̀ô¿åœ,4ÖZ¿ïÿ4`tAGNfsrq?ÎÁ}¹>Oœ?Äyëð9ʍ?ã%›´7:æ?ÉЍýë9?ĨuäÄÌ?¿kO"L«?Åj6Lõ?½"¨Š''?âϔYW£ð?Æ¥£x.?ÏWxP¸n
?ÁÀ'ôgå?â/ ?ŒC+?·†¨YOý?Ñ==ðrç?²•ÜN¡­ø?Å7…î
‡?¬2.EJ¨i?Ñ&cŒAl\?¬¹ò§X;?á ¡ÒÎ?¶郹Hç?É2â`1îå?«(`yþe?كH‰Ü4?ÉPUq»H?Þ¶G®Új?ÊI­µ§¹?¿¿%™†?¹SÌ-ɘ?ا9('x?Àînµ6Ðn?Üt'.ýT»?À*×íÅÉV?ÅÈiF?µ´Úæ§?évmäŠ?«àõŠÇsæ?ÁX*·ARä?¥îÜoƒÑ?±š¿%Z²?™Ómyµ?࢙>ø?©ëþ)0èæ?×Ûé*Ñe?¬ÅÁQɕ?ºƒƒFŠÂ«?šHœ­ÉrMIXED3FGL J0401.8-3144@lå7?1n7ÀHN‡à3±ÞÀ:V"ú¾À;ò·1Z?²åäÃ0
[@}ù?œx@J‡™xb¿è"Ûs¿çÔÔxñ6¿Ö¢}›Ǩ¿ë-:¾AïAGNfsrq?ïéçÎ?b;è1Vã?AѺeZI?@‡FÍó'$?bt© yéð?`0©×±'œ?îÎÁ!Ú£?›«í?o?'ìFÛø¶û?"dzVq÷u?œ±¸]ú¾?"î'ÓO5?íÁÈÉvÅÉ?šñˇÚ?š*>Q{F?ƒ4Êúˆ?¦ÎTAÎf?"Vëþ`?îÉ6Gî4?ž9¼G(¶?ƒ_k>"·?ÓÙþ
 ?ªû¨Ä#?š
ì«#?ïó0…7¬?R6 ¸ã/?:ÀÐð"ëv?4"N³jx"?RîÁ~Žö?Ng+j"?ï¥ ßœ?~œçÄÚ@ý?jkì'XëP?frmhŠÄD?€þÊÀ?v—Qu¢?ïµÎiÁ ?'À¿)¡f#?Šâ̅­"?sBZÂÀÇ?wßìvw?z‹#|·V³?ï…ÜZ¸?xw±+úa]?sò±+'E4?`À¢˜(ÿË?"ÆpDês?sRï%RAGN3FGL J0402.1-2618@kä}sÉÀGÓõÀjÀ9ø|]H°À;·ßâSG?åËWw"½ë@‡õ!ªŸ¦@ðX•m?ï2î>âi¿Üc‰¨ÆïN¿çÛ¸M
û¿Þ¿9€:‰AGNbll?ï²ü8ö?ŠÿWc"$?_&Þð÷ˆ'?c¾—ã0›d?&Æd'¦?ˆ¿YpDó?îm'¹ém?°[Rßk£?†šÚ_Š¬?©Ny|ò?£€ãéê'?ªãëÎûQ?íH '–§? 	$՘?ž"›²äÉb?Ô9+.|Ì?¬mH+þÜ?›©&ôCZß?çµÌ½ÞGt?¸uûa 0–?´`€'Ðj?°2ÖAÈ9?ÆøŒûóÎ;?µ­Ë¾è…%?ïЋü«•M?ª{jÐö€?D…uÐ%çÒ?^¹µö ö?u)Rò.ÈÎ?ªIt×)?ïunÖfBn?¡?'ÄÁ¥!?qç
2cò?ˆ«¼…!«?‰°ÈåU'€?šÿv³´¥?îëX¨¸µ?Œ5Ç}¦ ž?Ž=¨ùÙP?ãÁ´ª?"v)Æۘ®?"ä¦Ä`¨È?íÃ	õyû?Ÿ›5ru
?™´§çæÔ?‹À\ ô4?¦õ
!©ä?™ðÛß_,©AGN3FGL J0403.7-2442@kž¤_ZÙjÀGzX`fÀ:'ÅÁ?ÐÐÀ;ö2 f<u?¼#$Œ;j@ñÈS{½@ò`À48¿¾–û\_Û¿ë¡ÃBE°õ¿ÞýϦ=cZ¿ïòÂómAGNfsrq?ïaÿòT?ŒÄó7æ8?v"¯àý¼?zãÃFVË?ŒnÇÑì<?†°÷Bçè#?ë@D7VGN?·ýJ›"!‰?¬(dºI$}?¨ÝøD$8?·é«éO?¯Š¶%¥?êûVÓKl?¥'Ÿåµ'?¶@Ñœ? 4ká(
?±å+•|uê?—aÃu}^?èë×7›?³œ\x™?°X¶Œjm?£¢éðð?Ä$Hà‹4?¯–ž!õi?ï°±¡€ÌL?}ô€?Šja?g¿í'¢'©?m³#~ðV?{Ç8žº
U?uSè‰eŸº?î}DOÃÀ? ™§´Îú?"`æØ]O?ŽÏü9ôXÝ?œþRÀ±?—ý:‰Ûä×?ìדÚèÄO? šÖÙ¶­?°dôÙ'Æe?™¯	ÏSé ?¡¼Øl`F?Ž¯×Ù?íâ]昮k?"ÉöÞ¸?'0ÞRì?†?}ž…I}?£‰#•d?í- 'ÉUAGN3FGL J0403.9-3604@m·{€©Þ‹ÀH;Ã`<€ºÀ7/.g˜À;>K֘'ª@Žƒ¹Þ^@FG¤5)@¬BIхC¿â¡w¾ji¿è ×ÌOñ¿êPEҔ"S¿íÈ%?¡øÛAGNFSRQ?ï›ÍÆF÷?‰‹¸šZs?†
ç¼j¾‹?‰?ø®ò?YU&ÚS­Û?RÀäL `–?ï'
t«¬?+g:`sê?f®þŽ›x¿?|Q¦¶H?†£;dø+?"÷f˜™?ëןJ=?ªkh߶‹!?¸šº³0É?¦u\z3µ«?¡P™{Š¼'?™Ù45Òû?ïçófûž?u÷Ù©?9òÅ&9~D?Jæ±&Šw£?e¤´ãOÐ?t9€•5å?K¹?± ü³qv?€
‰8J	¿?Ž"^¦?ǶSå?°Ó³-
?ï՘˜'³v?rÑz!'n¹?Usªämô?TE·ç,àa?o­Ÿ!y:"?o:ÉZ›2?êñ™WL?±ŸRxðB?ÁÑgY;Â?«¶í
EI?§«»GMÎ=? C'p'€?ïú¦¢`?YöoÈ["?'-`' ÝN?5μ½ã??9:9R r?Xê3u?AGN3FGL J0405.5-1307@i¸ߨq¤ÀER3çüÔÀ9Æ$PA`óÀ;Èi;,ü¸¿ô/Þr¾"@öÉ™"{@Ä<€L¿âËK-ƒyz¿æŸÚ÷e…I¿áa¯Ü7_#¿å³` åÏcAGNfsrq?ïø"~//î?I­n]{(¬?…"¡'¹?8gw&2?LåV÷'5Ê?Hîï†
?ïèÞÙÈ;?…¬¬pá¿x?dR6ƒˆÈ?gÅ®í¶?†ñ:´>³?'+)Gû­è?ï#Pm'å?ƒ©lù_?€Ì=û¢
?gB¼òEù{?"/ÓSåàc?o¿q¾~?ﳪZ˜8,?x(Dãûæ?åä¾r0ü?'œ"hÌ·?'۝‹ßä?wÌ!õQßô?ïýHØG?4ÄçÕ^m?Çtwâ¢-?7»¶Sì?4,ÉckI?2ڇˆˆ½?ïÛ/AÏ?ixل÷ý?QÍB‹?P	š–þ?kêQ1éb?cu£‰÷)?ï®DpD›?cBÓ²ï©å?n{xåК?O)E¿¨Œ¹?y݊7»}ü?\Yî¤!
?ïòÿ"1?QH£]–ÌÉ>ùüó'…>Í>ö`<‹ô^ñ?Y™žJXi?Q8rPj&ÁAGN3FGL J0407.1-3825@n(*Á	J,ÀGìè_ÐJ0À8î÷™ÿñÀ; ÓµZ?ð¡R¥ê4è@õ5`Šz@.âôV¿âŸaþü¿æ=U?;n¿åp»ÝøTv¿ë ÂJñIAGNfsrq?ï؁½É"v?jSH`CÈ?hԎ'˜Ž?bÏ©ê€W?^¼Úä'?YQ9"ä1j?ïWÅE¼D6?'^Y™Ò¹?q§Ë-F|?~çp–ª?˜?Ü¢?‰¨ÝÀv8}?î'6ZÒUð?'Om¼Ì©?š¢³£Ïá&?‹<Ý·½$?"ÊÐ?€á¹¼üT?ï²ì`?–§®ôä\Ð?u'³€[i7?rК۝$?—åúùú»?"à"û×ñ&?ïï¼/¾#?Tbïî¢Ðô?V×Ý´í?NI"l4[,?Då'ÈGŠŒ??0	ý–®'?ïÀÕy³d
?vãÎ	¥}£?`½(Šý»R?^lÇn¶€?w6®ñý)R?qs>àW~?ï(^…"Êš?"*mùïûê?'-ÿiB"?*UWå?ƒÚ¥ÆH?n¢Sؔ^ ?ï˯ä3Ƭ?ufvÕ—?`Ή"Ù‹`?T¡åEž?qÀÉð4Y?s@•2âïdAGN3FGL J0407.5+0740@fý-`ûHÀ?)£?4É5À9\¨\ªûÂÀ;nNá£1¿ñÕ«}Ç«ü@Dõvºš@…¹'!*¿è®+£4I¿æ…Œ™"r¾¿ë^BØ¿À[{26šAGNbll?&ºe'?¢vƒûO?wËêuà?¡M:@NÁÝ?ƒ¶iÏu J?'i °×?ïjd£Ô ?–£ìc€?pXd³o?oK¨<?^Îè<D?°kåx·™?í-Øâ—?œëdþ·t"?¡.\UÔ8?Ž~ü3!Ü?«ô~lfV?"Ý¢e£¦k?î9èK®T<?¢@`ïTñ?L—'¨æÃ+?Yÿe/jŠè?«ïýÍÿ?¢)£`|H?ï»dw£Ð?­d»á*z?uûÏ!nmO?­a%ñ¶?h£ê%±>?i§fïtØÊ?ïÏÏӉ̿?u*`&wL?WÁf'ºÕ?]-yÜ¢P?r'¼‡Ý:ø?p2á	2ïB?îë'õû8?ˆ'Ǐ·r¼?Õ\¢®?€YÑy¥?'~ëÝ"R?}©YïwT?ï­K/ÜÅ?tS²@™Í?iۆþ ?€¸ –êÊ?"xù(.ú?tBˆ?àÑAGN3FGL J0409.4+3158@d–]¿Î·‰À,ÎRAtÀ9ÿ°ŸoœÀ;‡yÎøö÷À¢ëý¿‰@S¿[o'@û¨»w¿êX™|ÆØ ¿èžô'%Æ¿ÓN¦Œ-¿ã‹Õe"¼AGNbcu?ïÖÁŒþ?tc£²±÷i?F¼Ñ»Ì¯Ô?I¿3RÛú?qÇ܆&íÏ?r[À^?&?ïo˜ÝÏ?","/½?qœN®zƒ?yï0aT(?‹K×kw¢m?Çôìh­ð?í7•ÏÏOx? ýÍÙcÊZ?—~[¸~i?'Ý~iÇ?°cº'Š(?Æ:¾o?ïSßa`(p?ò9»ãp?ãqZrWú?ʎMëù?•y" ~_2?ìñk£Î7?ïð%tÃ?`Ú;Ô!>ç?4Ò8#;-?5ªŽ]"?Z|LÕ?^û'"¸¨?ïԘÊ"Ð?qËâþz·\?W^¶r?V?êkæ"t?oä­j7%Ž?kY;*"€0?ï!è¥ê0?ú–Ô)LÔ?''vJˆ²?iR?%¤f<?'°2§?|5}=×÷¯?ïÚß.E°?gÜ´èZÂ>Ö·w4	>áaý‡Ÿr?rŠºæë»á?gÚV¢Ìç°AGN3FGL J0409.8-0358@h{¢ÿ‰;ÀB¯Ø€_5ðÀ9n93't¹À;‡#µîe?ë\˜1e@WtßP)@"< DXŸ¿ÅéÊ A‹]¿àuñ—ë¿âÏòU¿Çx¿àŽ¬£ŒŒ–AGNbll?ïÔJË]êu?jÍàë·!?eÊrºêš'?a9.5L±í?eêÂh²?[íÙ&ÂJŠ?îÖg¥o€?¥-C¨ow?'r¨[¤?'ðö?œ£Ä93? ²³W?î@ÐWúE‰?—å ~/?ŸÏêªU?'Ùi–±,¿?˜óÍ:'?"S}J—tš?ëĝKTè?¤äN¤¡â?™©IóœJ?ÞÇ Ãø?»pÃ%rïû?¢õž9Qàf?ïçšÔò?`§>ñøîM?Z¢ð"ôŽ?W>//Tk¼?W<ØWGü?M.‡‡ƒ³?ïŸL
Ñz?ˆ¸a³y?jKM"ÛÛ?k¶uñìer?š+̡ا?"ÆU/‹?ïM£-ZðÖ?ƒA] 7Ü?ŠJ8Jƒ¸°?ðMÓØ?'Lü[¨kÈ?i.–>Ù?"¹¨$?ˆ¬f/FÚÿ?Žƒ2D¸Ñ?sŒ¾
°fÉ?šbþöí?""wÜ_±AGN3FGL J0413.6-5334@pm#@ˆÊÀFR ÿ¿h`À9:mæÎÀ;¼À2Š–Ç?ÒGp²D¶=@¹Zîu@Ïâ_[/Q¿ä"9¿äEÕwŽà¿éH0s˜ÜŽ¿Â‰,2§¶ØAGNfsrq@?ïöý4ÑC?I…uVv
?2ÁD†Ái?2'ôÀx¬í?J« –!T?DxE!š—,?ï¤ï7¾÷?'VÌû#×à?`À2òZúÇ?c"=Ç"ID?'"%t'Uª?~'·Vû.?îãÉAc2æ?ˆ¶92\»Æ?Š^·N?w¶H"A?–W|'h°¶?'vGO#?ïèóC%'?m¼8ýÓ$?0íφt?䑢ÕØÿ?f³ù!­q?mž?ëUB?ïüjäÐ?5ÊZÁ*ê??"ºãÆWu"?ëTä",Þ?3QÂ0Üúä?1='[ñ¦?ïÝÖšQ?kKڀø?P•6ìyÞ?Qa–ßK?ißR´£xO?d=$:×HO?ï'@®@Ù?t¡%ñØ}6?w«íÇÄ?b¸Ççºñ?€+þˆâ?pÀñ=—ªŸ?ïý8h¸al?Bò2¹Ü>é²kg~ˆ>é|áÕ¸?5o(«g›É?AÛ§;c¥>AGN3FGL J0416.6-1850@jÉ{¼¾bÀE/0ŸÚü:À8þ,"	7À;«kÙlî@¿¬=¨7•c@Á'eé>@¸áß®{Ô¿ä€ÚB×%¿ã
–t 8Z¿è_
Úyˆ­¿áEÀDbDAGNfsrq?ïõÎ.)f´?JGAA‰¿?;çCè'v?9刪8ñ4?K?Tb݌º?B§cÙÔñ?À
'Ì?‡=a(qµ»?fþI•žÛ?gôïº
[¡?ˆX‰+±]?ƒ¾[†í§.?îñƒä·¶K?‡8c†¨ŸH?‹Áá(§Ô?y©˜^íán?"I¢xtâ©?€¿ª?ï›@}sž?'yå j¬?EÁÚ[ýÁ?GbönÔÙ?‡ÜÒI%O?'=6
ݖ?ïü=/
?6Ó?ô\ì¿?$?za VÈ? ïi•.Õz?3÷‡Þ?1cã–#†?ïÙø<oÐ{?n.D̪§?R&I;~d?Q;Úö?lôžñDíÅ?hm>T¡t?ïÈtùQ:?qÉv᝼+?xÿà.V:+?híèÕÖÅ?å4èë?e‰ÙŸÑf™?ïìûo¼?P?b^îšIdD?$t)ú"
‰?³ p;‡?a½Mpî?b#¦,·ßyAGN3FGL J0416.8+0104@gúŸDÔEÀ@"п "`À9‡Ûk=À;Wè°X"ÀþHDè<@0:/{Ä?ûë©ÿ˜Q?éW
¥—̿仝‰'&¿ÑmE;Q¿ÐàP7OøfAGNbll?ïó€i-&e?P`ď¶?-¦T!giv?'O]§U?UJb«šÜ?N•Gì)\?ï–óbžìÑ?‡›°¯'¦Ò?eA	Ê?rô†óW?"òLj?T)?R+ƀK ?îÝ£#c»?‰®8܉?‰¾Ê:Å®?wÉí­k«C?—~FˆÎ»Ò?"}¶y @?ïm¶^Ì>2?Ž½Ä«œú˜>áý»}_>ø®·>-?'GF'W?Ž»Ø6L3?ïùÏÔ5?;󊡡¼ï?*Ô¶_¹
?$­WVË=?BËÌ5£?5 ¤º%É?ïÛá̍E?lƒT\qË?QºsCš³?Q(ܵP˜ð?k@ùý¬óy?f"L†ÅoI?ï€YUÞ?w<–"ò?{—zœ‡—Z?hÿû]¤æ?'í_—$×?q¶:£º»Å?ïß.iýq?h3¦¬™Ôç>±;¡ò¯Á/>¹aÅPü½Q?pg·Õ‡ñý?h3+˜¸‡ÁAGN3FGL J0418.0-0251@h€§ayWÀA"@f!À9#'RÑ^À;‡JaM!ò?ïÇã_û,@=×{ýQz@¯'ÿÏ-¥¿ç'üÏ¿áçй–d0¿épN[$O¿ïÿݹë.ôAGNbcu?ïڕtix?o#‹Â`Î$?n-LG¸ò—?lpëDCJ?Löa.?¡'?JÃZ%BC?틇Ò©?­Œ(êE]Ì?™	û!?«b"Qe?ªÃŽ>—v?¥?µÈZi†?ë}í­(Rì?¦É°y	J?ºõ­|áŽ?¢9ñÚ¡—W?¤9ҁ*?'E¸d?럍fxÊ?©õµ¬Ó:Ù?²R"ˆªë?¤%êÑÍ?°±æo\Æ? |ÌZ;SÌ?ïçÞª)_?eæ¹@֚c?cÔhJÛ?dˆŽK¶ ‰?A6R™ðlµ?='ºpèQ?îöÍ?ŸŽa?"g"•ó¿!?Š96Ç¿?'îc| ?"#»oMö?ŒÙC2Ä?í^¤ôt9@? †'m—n?¯|2‰ø¹P?œ|%=ÇÎÆ?•2üZÉV?‡è2ºÚŠd?6
u?'"}!#ð?—a'ò?"â	uK¾?'ëz­ˆHj?‹©áÿþ—9AGN3FGL J0418.5+3813c@d2`c'À!N·@§[À8סíûñ~À;4'b"s?ð`ãD³c@Ðü&Å£@K7GMœ¿çՆGqD¿ëùt7	'¿èˆ¦0š–^¿ïÿÒ"¢kAGNrdg ?îP›üþÌW?«ŒX¸O?‰q["Ó?‹Y}"Ub?¤™énźÈ?¨ýeà?Ö³˜(*kŽ?Ëj'‹Ø]?Ò,mž`u-?À{Û"zÿ%?×ú8b>†?Åm糜¾×?êvûVop?¬©Ñ'€ç?¶ö¦?£[Ô1Þ?µ}Y'^[Ù? §¼†©]ú?Û¬å]´³s?°Þq·h¼¡?Óµ-%þ?±Ì™Žª?Оu&6?±cÔ>DÚ?ï?û[^(2?—¼EÚÄv?E°*V?~°ÏôP´?/(‡i³{?"h·	Ó#º?áäÀ† ?˾—úKúÄ?Êødj¸°‹?¼;XRžÕ»?Íwhjøq?ÂÜ©'šè?í©SsŒY?œÏî?¤Èú]¾G?'Wž~Y?¡hëÕÇ4?'¶«ÿöæi?æ"ÒÒlÁA?£±6?ÇKËi)˜? å9ùG•p?½Aҙ{¢Ê?÷Ä>«-ãMIXED3FGL J0422.1-0642@i@lÚÀBÛíöéÀ9®°E­‰À;¹V¢¤W?易 ûðs@Õ˒@Q†Àyt¿àÖ.½Ø"*¿æ){þS-¿è§´í]&¿äj"]Ú£AGNfsrq?ïŸË/qeQ?ª+ ÍÙ?€jÿ†=0_?~Á'»äw?nˆÒ¥Àu§?fªïsmó?î#œÕcIQ?²™|ˆÿ¨?)ŽZª?¢[mË×-?¥±k˜5ˆ¦?ª]n}ޓy?íÿ¢†
†â?•dlfd÷?˜ƒÚ ºŽ?…Ämôuf?£Ãê|Î?l.5ú62?ë,Ƽ+X¸?«hýêWöW?¨Hȸï^î?œöÒnr/?ºueÃåXÆ?§çîØõ±?ïè}àU•´?cùå7"qb?[{Ûz²÷*?_$R
t¢á?Sˆccï?N¦±líCŽ?ïh
‰;¹¦?•õÄüç?yel·Rƒ?…šüÌíû?‰IçYßÓ?Ž¡¼22È£?ïLˆã$8?|oôþO?"ñ‹ù4?téJÑqb?ˆßS÷Ÿ?l™3éI¯?î¬ÜâHN?Z'FK?"ð½5ã¹9?|•ÆÅ.š^?–s¿qBÙ?ˆ."'EGAGN3FGL J0423.2-0119@hi#ßm¹AÀ@5ߵݝÀ7‹@ºs,À:îﲪâ—?õºX€õ‰@%@ô¼Õß@ž`‡)T¿á×ù}Ò59¿åwGø<<F¿äÝÌ_¥¾&¿åÃ'Š¼ÂAGNFSRQ?ïìĚx´?[õLëóa?&¤Äüø‹î?!Üјjé?aÇê&Q?[^"á%*Ñ?ïŒ<×ÕG"?‡ÞI<ƒÒ?f™6³ tã?s>ˆ¸'?‡J|m<X?æ>•v¬?î°º+yD?˜y<ãÓR?ˆº¥V0ü1?´âú^(? vW'T?"&"ŒC†?ïŒÝÖVÜ?Š$ÅO,?CHqS
©s?IßHoû+]?‹ÈAv¹±?‰ìkzVÆ&?ïøªümyU?CEüKQB¤?%k«uE €?"8v``x?Gù$s+`?A<óŠû¹?ïÕ-b¨…Š?pˆG©æ-?VpÞgén$?Tsqej·]?oš.a^·?iDŽf<,$?ïd¤ÅÇ ?'`8µL?|Ï3E.Ò?jŸÇ""?ˆ—ý9˜?~ pè'R?ïᒏ—À¯?nÚג{ªµ?<]]96×?=K:R¬?jáÄӝ)?nK³3}î´AGN3FGL J0423.8+4150@cöX@žUÁÀÃßé47À8MQŒ»À:Ú¥ÉRÄÉ?áE9bã@«ØW—V?þC‡¿&›ö¿ä™˜¦eÁ¿ÞãÙ5¿ÌOąÍ×0¿áS#h¹0AGNbll?íÙ<rÞ*)?¦<¤ò¤]ÿ?'ïÃê?'!<•y{?­°X`´ã±?¤8Á@a?ç	ùØÀî??Ê©Á'ÊRÓ?°Û>ß^«Ï?°+¨ýè?Ëjy+Ìà?Åîc—Ì\\?ét])HE6?°o?ž"Ž?©`]W±Þ-?–áÛ®An?ÃÖtM†_?«P§f¥•??ã'f¾"¿"?¹lŠ÷Ÿœ?p'‰ê?–ZÙά›?×$0©ôŽ:?¹£ 5vý?ïKÀ ·?"1<¿Í+?j/4h—äþ?eæ>€ËÄÈ?"BkzŒ?Œú¨vXZ?ìO{5Þçµ?À¸'y–? îbM÷'?¤#§ÁMÞG?µõ(ÅøÆ?·Ûÿeht?í9þÀ~¤?¢G›:§s?mšH|VÏ?'zÍ^i®?­©FÔ³rŸ?œOÜX¨Z?éû¯…·?«T"£
_?¶d³Ù˜?‡3¹ã2Œ<?ÆM,%ar?©H#ÓkbÕAGN3FGL J0424.7+0035@h2¢iÀ?Ëy`>.9À8'Ld\¡À;Iû_‡O?ÑïdöyÄ@üŠOú"0@•?æ¿Þu—''¿åsÿ©÷h_¿àSwa¥%¿ë/ó
åAGNbll?ïöØ®¤»?F½rÔw?4}sVt˜?/Oüs;o'?J^‹HZìŠ?B¹——éÏo?ïۂzÌ­?–×4ÀãÓ?{TN
JîÓ?w—Ëô—ºo?–Ï|3ë"?"ûy	`ŽÒ?î;0'2â?˜à¸­+d?ŸYÏÄö÷?'ÒªÁÞR?™C*æÍBØ?‹öÐ.ë ®?í¥UÓ#܇?ˆfìH=1?|€—éò?wâfNU?±©]ºxë?œar	'‰?ïûN"g?:"6	¹7?.Ë/Ø¿ö?$ª¶kµ"À?6ë°³¾?4Š$AÓKf?I­·Í?"8',‹?kÛ9"þ¬§?eúfº©q™?dß=Ñd?€ñ½m~!?ï$Q²
?ŠˆNÌ"®?º>ûtrF?…¤~)Dª¦?…†-œ"w{?{œv:ëH™?ïR=p_Û?'(4d÷?hÇÅIsX?Z…DÝ?'ŸYMÙd¦?ÀÇÑÁAGN3FGL J0425.0-5331@pbâ:¸cÀE€ÇßþùÀ9gCÁðÀ;ԝñ.ñ¿õåØõ$.Þ@Ùð5²"g@®ˆ  ^…¿ä¾è$/ùÝ¿äÔ7r2!¿ÜÛpí0£¿ëãAÄלAGNbll?ïŠËæÁë?Ú¶
ÉA?~Ý⑷¥W?‰³¶W=Ê(?{¼"&tå?Ùlä¼W?ïWáõ˜??¨À¸sLÉ?n'<êLœ?n¥œ_¤Ý?'>ö6²×t?Œß"™ß
?î,ìXj?™ì6Ì$CG?¡ZÎ¥Š?"+²z*u?šÆä¾K£Ä?ˆz×Û Y?ï7Îٟ÷Š?'¶Oª.´–?SÑøŽð¿?c¸¥'Š,š?—ɉäj¯?'Ï q?ïÙ¦«a?svIyÉU?eoÊJ_?mÔôNöý?a%Ö%|=?bâW1ùû?ïÍô½à(}?skZJèÀ?X°	<˜?WäÆS?rÙ}âêR'?n—øª*F_?ïC±µU.?…ù¸ßæø?Œ»òÆáT?œroé±Ý?'WÆů"?s\¶5À±?ïÖ `2DÌ?vÏ«1›%Y?#j—ÖÏk?)
'¬³Ä?t{Iá"?v¶"'¥wAGN3FGL J0425.2+6319@búâ~@#…ïÕ"\À9Â*·c®üÀ;röq?Ù¾9½w*•@Ì~ ïÏ0?ÿme¾Ë­=¿ã—vå˲'¿èç	<Gaœ¿Üf9±~N¿…è¨(0ScAGNbcu?í°«6­™´?¾cPK5Í0?c´éOf$	?eˆåS˜¹¹?±Üÿ=º?¾J@ð$¯?îwYö
m?±B_ôºÛ?~µõ–¬Á ?'c
£ï?¤³¡íûñ~?¯»DxЭI?íìë'x6j?‹0Ú©O?øèô¥?¶>
g»
?¨´Ù
#ß?™ ˜gD§?îšÚð¸¨?šo+øO‰5?Zÿ:2Uè•?gÊR<ŽØ?¥zW&Zò:?™Þ

eê?îªò\~[%?Åk¯•H?ú?Qòò§"M?{ƒ¹0)gÔ?¤ÁB¡'t¤?Åh±hÜý
?ô[¦?ZS  zÞ?dXíÑX
?bþ¬´L¤ÿ?"Džœ(î?Š^6ìü=?ïIß
x:5?ƒ»K…»q€?`²çÛ0g?vÜ	KÈFP?Œ'Š†ÌÐb?~†	wؓ§?ïµÝÜáå/?tjK²_Ö?P¬/µe?P@øüª-?€""?
å!?su:€ÃAGN3FGL J0426.3+6827@a"¦°)(@*°°|À9ǾZCBuÀ;£°Ôcš¿ñ·O,´@ '¯€@Ò@!¿ã1i¼¿è3©a|‹†¿â'7Ín)̿䈺›"=AGNbcu?ïö›þ"Û?³f±¡Š?f°‰é¦?x|¥"ÁÀ´?šƒ•š]?²‡‡Mü?îd|ÉK°O?²TÔüBǀ?€¼õ,}
?‰"™ÐK1'?¥Ä/…®Ê?±Wð¿H¿\?íÝëÏá"?¢•ëÚÇã?Ës2&Ä?zâå,0ä?ª.b¡²X2? vR"ÔĨ?îÒýʵ_7?'Ne:WÄ×?U(‹oÎZ?QÿŸW}¦?¢(>Ê%?öƳg§Ø?ïLͽÚãÞ?Án˜nÌ;'?Nº—Ü2à?y.Ä!¤2Ù?•ps…ˆÀƒ?Á>µÐåi?ï³\8?'sÌ
[Ʌ?b}òe·æž?`Åó÷?G?}ê\ºt?€Cô­+¾À?ïRÀD†Ë>?‰Í²ýx#C?y–…&°š?^·Œoù°Û?Ž"æ*Ø ?ˆ"gåô9n?ïÃðÝD¶‹?i—}Pñ?1舚Z
c?(3Ÿtî?|éÙùŸ(?iK5Î8ÅAGN3FGL J0426.6+0459@gµq'lÀ<î™?׆dÀ9RöT…"À;T"K"bÑ?'Šò˜Ö~'@°Ü{š*@q1ßöö¿åxŸú쵿çê_5UÞj¿æDªøÍÂÒ¿é>!'}AGNbcu?ïâ²sž÷ì?v(͆â"?O¢k*•‡Á?^xw´7AÅ?edñÙ»	Ž?qYÒ՝§?îÿK›'? Òw`>—?|Îx_îkC?zúy"|µn?˜âÿ‰ÐˆJ?Ÿ!JîßÉ?îÆEØ?;Ī©U?Žøyç"?€ùü:¡®?—»Dƒ;?ƒÔh—Ùþ÷?ëÚ8ÿ²•?ž¿­ðâ­?Š"íú"½?{jTY¸Ÿ?½íçl¾Í¹?œ|¯º(–ˆ?ﯤ2yÏÐ?±õ§š¢Óá?Z™«Ï/Š?'Dµ–Ä4õ?€Õ - ?¯Çª¿Þè?ïªsiN¿?"ãâSvéy?gK
%G¯6?fŽ{ŸÝÒ@? Å
¡Dº?'#.x¤Y¤?äðì?x'¨Pô?z°.w\æß?k0u1f±?x/¼Þ#¬?r$.¦c.?îÌõwÌüY?³É{ø‰•?tŽ ûŽZd?\[rÑà†3? žÔdB`'?@ÿ5=;AGN3FGL J0427.3-3900@nEg!éBÀEöŽ€`ãpÀ8»rƒ«ËÀ;AHð3Ú"?æ"Uö_Jò@¿%oü^@`;»²¿áÿfyJˆ~¿éç±(Ó"¿çµ'"?W¿ïÿGýUçÏAGNbcu?ïùõP;?C)V¨)*
?3Ž® ®‹?3ûMæÍÆ?B0ÕSýs?<#B	&f?ï-'×!~D?•XsMnb?vóº4·GK?±‰ZQX?"¶•)§¬?ÏTê Å?î]¢£i¸?"ª`×­½?œØÀ²…2?Œ…¦š?—‡*û-Ä?‡ÆªZj?íC¨³â˜?¦iöV?ˆ5r+*K?'È}̨ç?²Ü!·ºá?¥&¯ §Zñ?ïû¾ ±?5ˆ»¦Gƒ?,o'…|½??'8Ω³Œ(?3ØVm€?*÷Êx4a¥?ﮆ¾ÔP?}4ß»­:?fKçæ×Ü?b£ÔߜY?}uú¶"?w9‹"£«?ïÈñå¤Ï?"Ê@¥þì?'¯OÓ ó?{æÔV+J?ˆo%EÂ~?w)µo[Ø?ïEP™AýH?†¾—ºMA?tZÜ'WY?fÊн*?'?5Ð…+?…PU?èòIAGN3FGL J0428.6-3756@n‡?úÁÓÀEÏàaÕÀ6jˆû¼¤aÀ:3Ám9Í?ù˜ðN²»@õØ •ŒD?þe@å£]¿Ü},ÈØC¿áC,ú¨¿ßì>{¿äŠI2à
XAGNbll?îÙEë`zƒ? »ÄUž±Ë?F@ö–§þ3?F¤FȨ?¢pє×? ›'õ4ÂL?ïž!@õò?…nBT˜›ˆ?aÒ>=âÀ}?dɤ£1Ï?" 7Ú?-?'f_<Fô?èL!':?µ&.çã?¡cEÕº@µ?—O¾yA?Êvöî@)?³nuíVªé?ïä‰×ڜï?vÀjÅAýI>ø><8+<H? '‰Â¯Aõ?kE«½&÷D?v¸~¢Ïx¦?ïA/JEs}? òÝ:Ä?@3ÉX"6`?H¬XkÁ´?—Xxgê? Å@Š¥Ì?ïÞ\
¿R³?l$÷$öïµ?PtçGGH[?Q¶•eê?ii~_0±?evUwKÖ?ê…Ž°î†?³âª¨·N?žšÐ©ºÉÌ?•¢·ès£9?Ãҏ±…Àì?±«iºS¯?ïø"@¨Ög?XHÐ&â>ò!øþ4d4? —;Eö"?M!ìâ]'
?XŠë8AGN3FGL J0429.8+2843@eG¯ ×{|À*ôUÿøÀ9¹õÞ>YÀ;W'2ÂÊë?òÿÞÇöú@ZM{³Õ…?ÿiE pÝ¿ïœø¦ÅQ-?ít:!ín6¿ÛÏY*Nï¿ãf pMoõAGNbcu?ïY
•å
?"ü"m7U?"=‡Ð¼l?…àfš"IR?…÷¡¦·?Š+C¢,•S?êæ5§èÍð?Ä
a,ë›o?®†ðڒz?±2á=lÿ?¹ŠÚ³!½?¼ÿ½Øñ¦Ô?ë8»áÿA?¬ÛhñÛúè?±Úzmèî?zý§T%?´_¦Ñ?¥èEãÆ?é&¹Sb?·`×9?ð?ñ~Õ?"r?´õ¸5Ö?®Øi_Í?©sšwØ,?ï¦ö5É2?˜Åíå•(m?vØoæ֑?ˆ+^.‡Èy?u¬uùG?Š/5ÿi¢É?îÒ Ì=Ü?°kjd'?—ñ^ró>?šXhíld?¢
&®]¢?¦9}~t¾Þ?î2-• ¡Ý?™Ĺ¡Ú'?ž:Ú{Éëj?Úf6—v?›rNJÓ	?(äVª|X?ìÏüD^©¯?¡{Í'?´" ôÇ–?)µ¤õ¿Ì?•uó¢#«×?‹‰÷%–žAGN3FGL J0430.2-2508@kóóà7ÝÀD "?Åè­À:•mºîÀ;Ï¥·µ
"?²v_ÛA`œ@­•ÇÒçï@‹ïà"?¿Ï#.LË¿áR»<	N;¿ç¿oA+n¿áq'ÝëXAGNbll?ïïåx«7?X
¸J?@ðéBÁt?AÐVP$d6?W½…ü•§œ?Tœ'®'â?ïU«
ZKü?"»Õ‡i=?pMÑ\8?}ÇtIá?'7*Uí\	?lëRÙG®?îãи¥ß‰?‹347¨?­‡|N?¶Ÿá÷Ÿ;?"m;kÊ?€‹*¨6 ¿?î‹aSñ³{?•Ã®b_)?sÖíðØJ?n˜êØý?¤Ï
!"<Ä?•Áv\œœ?ïù l"ôa?D—¦wÙZß?+¸P=Tí?-ÄéI÷B1?B9ƒ
_J?@6c"`™Š?ïÌ%½©Ä4?s†º°0?Vû3ªã×?Q$¼Êa'¶?t.Taa/ú?q8Üg	ÿ|?ï~'µãj?{9–ñ"ìŠ?äaóâP?v³‹"ÄOš?|õá(±r|?e±Æʂþ?ï·S*/»?qôö¡¢?Vý‹ÛdÅõ?D¿Måfx¼?~¶óSf?p;kx5|'AGN3FGL J0430.5+1655@fxV[åÚÀ5ªKÀ9B«×‰¿1À;NaŸWH¼¿á®ÅÁHh@Ò&Œ'@6†@ €¿äêG‹H·Ä¿ìRþ]Ï¥+¿ÍéY¨ñXü¿ÛšÝl"AGNbcu?ïñ¨q×;n?Yc"Þ›\5?%ßñkq—?"×ä!îÀ,?Yó¡ÿå@?X¨'F `¦?ïyºˆbÌ?ŒDÕ&u{%?nÀ¡j{Mn?tÅ
hÅW?Š
¨÷ñÃÆ?†®ÀZ>3?îšK%1,?"6‰•D¿/?'"Ñs#²è?lÿÙvIÏ?¡¹–ð4‹?'ü62FB?îÅÍXk…?'ØÍ	~F?+œ%a¢?1+uüp?£'g^'g?'…‡=÷\m?ïø'۞?Gl|(šË?$'Ñf­? Ú¼y@|S?J`Þ¤ Ð?E¶E‡D+?ïÒYˆÔǺ?p6°–åM
?W.,^eå…?Skó,€¼&?q°l$±‡?jz‹‹!?ïjŽˆ]Jù?…UhÂU2^?q÷"ÜNª?`ù)o5¨?Œ`"q??"­–™ U?ï¼(©á÷?j]Tø^/?#>þoÛ-?]§É«°?€©ôû4×?j4î+¼¦AGN3FGL J0431.6+7403@a``þG™@1\w·À9±{£aÀ;¿Á§ÕœÀfºó±h@
±Šî0×?ÿÐNI¿¾‡*…~sg¿ãš+Œ°a¿Ûf¿ÕÌ€¿Ú@`"ú¯oAGNbcu?ï´:†RƒÊ?~MÚI$E¶?YçŠäX-?Uꍶº!\?Ÿ'ý£ìÈ?{gGª;?ïzî!Ü?•?s®?sz¹Zrc?'F‹pß*»?‡¢§ñ\_c?'¥E…oè?îVƒÄ4Ã?–›%
jF§?'hˆ›Àþ?6ɝôÄL?¡c¶w]?'5<ࡏ?ïvÌwE?‰ÆéÝ–¨?'bøtõÞR?1¨èÜš?'
€}0/Ý?‰¦iÚ»Ø?ïâ'ev/?jp•ß»ì?P‡7x±|m?RÃÌ2Êñ?e*ÿ•?dTx´9š?ïØWHÕö†?tIÝ1/‹&?Z3\GH?U?}ðKý?jþJ®?q–æ4G]?ïdšÒåѽ?yÃòԍ|P?	¶M1ž¢?p++ìÞ¶<?…Ï"þ)f+?oféÈú?ïç•}!¶+?`@Xäó>ø簎­4î>ÿDóv~ñO?h8³^<zr?`5mQg}ÊAGN3FGL J0433.1+3228@dûá`؇ìÀ$Þܾ²W×À9ôwa`m(À;ûý<a¿ÛM¹ë¸d$@eýua+?ÿ~5?|푿äq#mÑG¿Ö¸ŒÃпàDe°¼~¿ÊÛk‰n†ÏAGNbcu?ïÇvåvù?uú¿•&ü?JÇ<Ž¢¥?E*‰ê‰ˆ?xëЋ,Ë8?sÍ{l‰ e?îÍõ˜?£¹V7d?wò_õ.Mð?|éA)? "[,sô?¡k1O£ïB?îÆɔ¢Ó™?
tÛƦ?‹›Ð÷?zîtÄxl…?™Xäé;Qí?…`˜‰2Ë?ï/˜SÉUÊ?†s(UY"É?Asã¼E•×?C¼¤]ÝHÍ?™Vp"Õ¤?†LŒŠ7]?ïðLc°Ô?TŪެCx?1ñ¡ú{¨Û?%
5h§Ù?ZdþBùÂT?SƒE‹¼]?ï'r´J?' &ŠX?dÚ¹%!`ò?hÞé)Û¸Ñ?†"õ=q_?ŽŠÁíÿ* ?ï…@¶uêµ?uê'ðSÈQ?zA,ÉÎFö?l2êÀØÄ?;ü–M9?lʘ4¼‹?ïÔªÚ^±?`j9§r?.W	Œ
i?$§ÀÛsI÷?u
Ôá¸$?_ð±!ÛOýAGN3FGL J0433.6+2905@eQŸÛÒúÀ)3UÿæՍÀ7胦MàÀ:ÑñËu?æ(Äwò3@Vmrõ@+&`;ÿà¿Øk®h¢p¿â-ôT"¿à+=ðÈÌÚ¿ßÎЇ\$AGNbll?ïöú
ÞÌ?MÊö¥
«s?&K E?-g"ù•?Ns¡^FHÅ?K3ŠpW¾?ïY[h±oN?•œ…³èã?pý` ýª©?sóm¶û?•:ãvt‹?"µEÞ¾¥?îEÄ¡ý
?šéd«çØ?ƒzÛx?‡
uÀeÐ?¤<^ÖÕ-Q?–"XD·*~?î·YºuK?–¢³ïgH½?MeW"ið(?Qð¬"¤Å?¤ÎûóxU?–‡Cøõ—?ïû|!'†Æ?;ÈȐI—À?$(ä?^¼?/MòÔ^ž?:dnŸÍV?3I}E?ïÅ5"¿ó©?|ƒnpá=—?\‡‹MÉ0?X4¸!!ÁN?vCRÂô÷ƒ?xrØuޏ©?ï÷…÷À?'ÂÇT+À?‰G"†bÄÁ?‡òƒió?'X6ÏAš?‡Ê•/¿š¼?ؼ´?ssþñS¿?F:DÒÓ5÷?:éCËwm?…®¥‡sT?s5ãœ\•AGN3FGL J0433.7-6028@pí_ôöÀD'ï¤hÀ9*ÜÇÔÀ;É'o°'?ãód»|ª@æ'M@–?Çì¿Ý&â k¿æ$³­ZÛ]¿èØ7»x¿ïþÏë݀œAGNbcu?ïõUcb{?Qçz†ÜŽ?Dà˜ÔÒþf?Ev–žV~Ê?EÉj!"?E^rį·Å?ï{≢?‡Ñ'ŸÓ"?j•†
*Ü9?k{‹ðnR?Š"¥ß"&Ä?"|X@ââ?îIê©Ewó?•°AÞu? T­C¤?†ü–»"*?–PUzRN?†…£Ûvdµ?ï¼K™Ë1†?(Ad9ÀŠ?[œ-:¨?bD¡½ýî'?{¬or"?c,÷º:?ïø¦}éËò?EK-@Ñ¥?AA4&Lˋ??sÃ_…:?8I¦k@Y•?2þýJ¶T?ïÏCaKõ?s'®wþ~?Z6Éÿ1µÅ?WK0WÇ[?qМ¹¬X?m•‡Î¯gÅ?îñ'¢W?Œ&ÈržMË?"òv|Žª?ƒl!­w˜?‰¶r˜Mê?.§E‹?ïó¿ëÆj¼?`F¤P*?<އhlƒ¸?Q'âJj?QH†ôQÔ:?Z~vpÔ7RAGN3FGL J0434.0-5726@p¯ 6mÀDq™_·ö|À9óÁ¯bYÀ;ٔ¦ë'´¿ªù[?ÿç@'Ùv©T£?ÿú•ÀF+³¿ç;áVûi¿Èx½Òš'o¿äX"ƒv±¿Òé`VVúAGNbcu?ï÷ùÙ(?N0ð#‰£m?06Q¡"¬?0ÕĽ"?IlïW·}M?Jð‹^¾Š?ïz,¯
š
?Œ]Òw¥Œ?i2	œÔM?sí¿8Ž²?‹(Qã	•¤?‡J ñ£W?î¸U[ýò?•ÇEŒA»?Šb¡Í'?"C˱Ç¥?›Ä¨™à¾?'Í©Ù'3ó?ï\ùÆ·à?ˆC%Qoʘ?XJ\3vi?Y·5¨¯¿Q?'ØɸÎÆ«?‡¨éìãۗ?ïü¨Ã5ÒÓ?8]ñ!^ûS?ôà©Rñ?è¿Х?3<¯ùT4}?3t·Ìj?ï×~Š'>f?mË1'WY¦?SÉI½¿ºÕ?Sv'
*T(?nœÐÍæ¼Þ?g–ôTLqÁ?ïvƒ|̯F?ƒ
ßÉ&®?¬_mC'`?~bSÆtm¹?'ˆñ 9W?yic+?ïáÔJ3n±?cfœ÷Z§?;Ç÷¤¾Lö?3¬îLs?j²¶é'»?be~z%€XAGN3FGL J0434.0-2010@k8
¿cíÀCx–@HÅlÀ9×
bY'lÀ;Å
ÎÜd?ðz8ËxŽÝ@m³Òê@–!@l³?ïù\œQôƒ¿Þ³4²‡¿æõb!£ò¿ê#£7AGNbll?é†ÁŸ¿oä?į泹ç~?Çè9éõkk?āë˜ûö?Ëùm]´8?ŒÿËaC»?ê'(ã?Á7…ªpÎÂ?±PAì\?³Êß8"ƒ÷?ºq·N¨
?¶'ç$"/f?毋õÛӕ?·Å˜xwÚ?˹EÀm\¿?µO8;I›ï?³Ó¶EÙ?œ…oÜôâ?ã`ž%o{?ºg%Aò­v?Î5ÐãC?¶±¾‰v?Ô¬¦Lì~?³«ç¹ˆ‹?ì-yxšy?¿@ùÕ?¼gLÚ?¾û³Á8?g:ùZ‡Q?}ì)ôkZ?ír§ú|Õ¶?¶]2IÏ
?£=×ÞÆñ?®aÑÏ?¥—¨vØÙ³?¨簔7#?ì‹Óyq?¨6J-ºg3?¸Ç~ö~l°?¥_Jš3D?œ0‰ÆÎí?‹ºïw)?ëÅËø¢¥?§s/«?¶'š"Š?ž¨$H?Ò?¦Š'µ,›?›ÚøéÉ"lAGN3FGL J0434.4-2341@kć rѯÀCõöÿ¦=íÀ9ø*/~rÍÀ;Ш•µßJ?äèþ®òf@{'Õ‡ÜX@ÃÛËÍH¿à>+•ì¿èæÈtVÉ¿ãÿ©²&¿n¿ääµ
_AGNbcu?ï×ȚIS?oØx1T×?TΤKÁx?U¸¤:¡*v?mÐejhÙ?iˆR˜'ýi?î'DO)!Ñ?¦»ùT:?†«ˆg>¿?Y>G©ÛÞ?¡X-çÈ:?¡ÓÐO¢Ð[?îYB=+?']Ú)@f?')`y™?}‹N‡èÕ?¡W,)?Á?‰¯m7Þ5!?ìEKú?§œWž]Û?œw±]ù‰?'IÎÛ8Ù?¸ëB!ÆK?¤«­®©•?ïõu{4Ý5?Q`cƒº4œ?4è6aOS?3RÇìåI?Oµ÷NÒµ=?KúqŤË?ï"SHžÌ¬?‡<;sYr?l|bŒ&I?i´ ý}N?ƒÌRY·?ƒ¸g©Å?ïoUŸˆŠÂ?vז¬`ºæ?| S×xÞ?h•éâ`uŸ?…Ún2þþû?oô¦**±¿?îì6XŠ8?ˆ+Ô3`¥?:Q‡™ˆ?vL,ü$å¦?"âtÐ,?(Ðø6M;AGN3FGL J0434.6+0921@g^­@ªêûÀ8Ë@—ŸÄÀ9Í
eÀNÀ;‰pà<ìÀQ4MdŒÇ@&`ú–´@êè CZ¿ç™ØÕTìӿُW¿Ûu#¨¦§Ê¿èÔ;D_ç'AGNbcu?ïâôö{`¸?g)0Óïð*?Z.
ŽÖt?^žÈý'@û?_èCnµW?\2ÝgƒV?ïnÉKãÙ.?ˆ)ÌÛz
?rŠ¡Ð*?qE¯cÆ?‹@è
×`?ˆûøþ?îŸåìƒv?'B¢TÎn?'´8ðüÝ?†`Eo]Ì]?™j*HÜpa?ƒ÷$^	Ò?ï,<må¥?'@Ñᜃ'?;á‡&˜ù?IŸ€ÊÙ%?šçÛ6?'rê[½'?ïõb…[I'?LðêcD?A 0•h?>ÿÖ<ø:?IfÉW¤©t?Cvœ¼×?ïӟ	0?p"`À?ç?V4ºú>ÙZ?R—ÇG'âí?p£Lš;@Ð?l%¢«Uù›?ïtÏ2¶>I?}käÍC?€[œbß?vم€Ôš?'p—Dè*ä?pTH'?ïÊBs9ö?p&£Äʶ?x1!"¨ž?&Ä×CËí6?zå¼8?pòjXGòAGN3FGL J0437.2-4713@o«˜€"åÖÀDüsßË­À8¿qw; ÀÀ;Àîû.	@šõº+àY@	«¼üK@ø/M˜w¿Ò´JÀ²¤¿är>Y_ W¿ë·D)Јï¿íĬ妸fPSRPSR?'Rî(UùK?›_ÆÐc¤"?íN4+‰NP?¾7¥-N²?°ù£éé¨?¹œ±ú&ç?dzaä*EQ?yªeãP?ì!®ræô¹?À…
ÐW_§?¾N¹Xs+?ÀL£Ým ?º©'BÒë?¥Ã}isrO?ès5'ð?²ÀããÔK?ÂJé'ÊÊ?ªD/½"pÃ?`}®Íwˆs?bä"çu¾ø?ïkû_B–å?Œ›õuÝ?pÞ9†´e?Š1AÖ	ž?zJåÚwsÂ?‹	©ŒR?î;˜ŒJÈó?½®·ÛE'ã?¨ý}œÈT?¼Y€+ƒ?xÂ=.	)×?Œ]Éۄ4?ì~оQ'w?¼œ¸>íõ?º}V9iûi?»»Çýì:·?Â1QQx¡?©äì"FLö?ç:"!É³?±µV
§š?Àæ&(ø`"?©Ÿ3>IP|?­ö]=í|?s|8lÑb$?ï@9&Î\*?ŒУ"?
]úZ?…c'#PSR3FGL J0438.3-1258@j;4 -œñÀAª(CìÀ:/rq6¤À;ÀlÄNy¿Ó'èxWˆ0@ú¥>hp'@Ù f|â¿ÞAš»>¿çÒúdúDn¿°pN$XØg¿ëV°j¸ÒçAGNfsrq?ïæÓrF?díy/3ÑÁ?P;Ȇ:T"?PR$kú?a©æð*?`g"ê·¸?ïõk¦?–Áâïì?zž"0©°†?€¬	f?—ÔQ e?'ÍßÃàÅ?í¼46Ø?š?À½ÓhP?¡ªR>/Hj?'ÔÃï·+?¢š~c5Ä?÷¤Tښ?î{|‰N¯?¡¦ú(›AÊ?e‰$#ôB‡?oQm!•ÍÄ?¬ÏµôéØi?¡Cðä'â?ïð|ÖS?ys˜«Ãu?D~
IVçÛ?[¨æ…†ðP?UÀ1.0u?rYŽiuF¡?ï·8÷ÿf¹?ykP^r§?cÏæ!O‰?`H'V»‹Ï?z{ãFD¶?t*¥ƒ§PÒ?îãLr
Rh?ܶ;ö,?"c°Ê$á=?‡«¼¬¥,M?2ÀíQ™Ô?ƒÙ§ã¶D?ï'ûªREê?w´h÷>&3?Z4U'fÎ ?Pþ‡¥"\p?‡úŠ³_«?uê`l`€:AGN3FGL J0438.8-4519@oY._ú;›ÀDåù jn3À9?ÖbwÄ]À;¾s"LS?ëÅ`ûK@^d‡éîÇ@!¥?êüŽ¿â¿®{¿äpqÎ_°%¿è
žªÁ¿æÀVò!'nAGNbll?îÈ?(MÁ?›áœQT½d?˜ Ò[?•aþ|ç?÷ú(ù¿?‡Íݚ¯¬?í1
8Å?³;e šÄ?™ž
ǓÓ?¡–@™"=??°Gà&ab?®m­ú%?í7Ã*.C?Ÿ7hnÈD?¥0£}­ö?'­•?æL?§S*B mÜ?']ÿ4œµ?éM‹ž%¼Ê?²¥kç0!?¶Äözɉ?¥Aݯ˜ëf?¾Ï–¡*¡?°§r¬7.?ÓÉ°?€-ɽÔÜn?}V§Û<ƒi?x(u6hÀ?sfÈ/ßä¨?kÂM"í?îýŒ#Ô	q?Ÿ3£2%á?†dâHX5+?Ž`XiÕZ?•
h1ïF?—; ¦9vU?ïWY¿J>?Œ>QâZY'?'pÖ2¯¦?"Ò A®o?}PXu?y:©'åÏä?î™&Eÿ?™‹ÛsŒGT? ¡Ä¥$Öé?"™}Ŷ;?›#‹Æ(`?"zêÿS6þAGN3FGL J0439.6-3159@m"†_•'ÍÀDZ{Q^—À:fùû@ýÀ;ÆõPy•¿ùh80)1@ÅB' Ôa?üT}?ñ²Š¿ïý¨é²z€?ïýÎ'üÚm¿éDúöÄå?ÆÁOòlÕ§AGNbcu?ïז:9$?r9,u?Mí6‡T'?N†'W zD?pw@p‹íÚ?q
#´²?àÁ:6?‡wsC?e³ŒKĆ?r ©E™Ÿ?…í¤ÁgE?'¾0y²Úñ?î,›¯H'{?Y'äuŠò?"Qp´=ÌÏ?'.—HU·?£Œ¯¡#ï?Š2fíelÃ?ïÂÀȘÆÇ?€j+×o8??óé΍@?U™nò<Ð?|£`a{…[?€ý‡{ô?ïíñÜÀz?]!:jè‰Ê?;ßouF ?=•OBƒÜª?]Ì@:бï?Y<«7ÁÚK?ïÜ U†«g?iŒ:þ‡³?P§ãñ2?O;aÂÉ<?k¹3uGà?c³8Šõƒ?ï)}`d*?w¥Ô©#?†¢Â_:Â?sgÔd@¨Y?ŽþŽ(ßf?uvÄ+5\\?ïö"mQUø?Qy:uê	k>õ&ë|bÄ?ŸëqµHè?R¢ŒÜ˜®ú?QfYç*-¿AGN3FGL J0439.9-1859@k(¿;ê'ÀB $€	À9Õ~ŽÑ¿À;ª7Pþ¿õ'óžá@f' 'ìÚ?þµá)¦¿çÀØˑA¿á>š'LËá¿Ú¨—Êr»›¿Ý¸7´¢3œAGNbcu?ïôs°Y'0?Q'[¦Ø¾?-üM–Z*'?'3yözŒ,?SYªh??P7Ìýˆ3Ù?5M"³?†m"2Óé?e/¬\ìz?ecÎBƒT?ˆÑ‡—o	?ƒ¬6+"?ï-܅H÷?'rˆdS?'˜0ЏÊm?r^ÊOiÖ¦?',zÜ?zßáÜdS–?ï´PT+P?'àVÛ±.?«¦ÍÒ÷?ûÀ
µ¦A?Ý"¨ë‡}?'ÎŽUß(Ç?ïû1¸M©?;JVÈ? ¯m-Ä'ü?˜î)Wº?>®¼¥ÆÙ
?7¯%zæÕ?ïڋ\(?l¢[ñ ?QÍßCš?PŠ
À>?l´Ñú¨?fû)~ký<?ïœôVöÔ*?rÜÀj%Ô?u†[~ÌÓÊ?m鷑Ê ?{ÿxô›v?d31Ö-Ë?ïåÁ-sb?ZHœnè˜i>þՖ´øT >öìeeÆ*ý?j'ò‰1.?Z+Mʄç:AGN3FGL J0440.3-2500@lT2TçÀCÿ·äÀ:ԕ(ñÑÀ;í(åÒWP?êìãZON>@yAôl#?û–×6&-¿ïþ~ôãÓ`?ïþÒúb¿²@gÏ2f¿éölš:²AGNbll?îjgê?°c3ŸŠa}?£ãF1Õ ?­¨!ðZ4?…Ó¬Û'×'?Œ	ÈõŠ'¼?Ú[Ô¸º­L?Ò¼&p?×!XçLÖ?Ðî¹ôÈ?Í%ܼ½?Áw~ôt(?êÍñØþg?°"õLÀ'?¹6âw"fM?«ÒÞb5$?°YŽ¾Á"«?›®¼(€Jë?çÿÁ@I»?ĎØ?ǖ,?ÉÞò¥_±¨?ÄPÓUÇÄ?¨ˆ!_Õ½?¦?[VBj?î*¹âVË?¹QW"¶?¥^šÌèš?¶]
³ÆU?×+æªó?›nŠÔ@å?ãlÌ®2Ǘ?Ð%«õ€Žõ?Ñ/®¦ˆY?É÷o¼ë2?¿ÚàÏ¡á?³\ƒvˆº?ílQœw;î?¢\BÛxµi?ªÜÂ×35À?žæ#¼Ææ?œ¼F½Š¬Å?Žµ2'?ìlLYtæ?¯)¸ÞsâR?¼GUÌ\²?®›¸/kYi?‹'²BÑ?ƒH%ô1qAGN3FGL J0440.3+1444@fåw'þLÀ4zƒ?»òÀ9WIáËa"À;Ip:$¾ü?â
!÷N@]E€gÄ@(k 7™¿àh•ž?ú¿æn¦ü®'οèºçC_j
¿á ¢Ç둉AGNbcu?î5,P"
?¦0–Ÿ	J?š:)£eÀç?›ÜröÜZ?Ÿ R°Ñïv?š¥l:Úª-?íÀ*äz?ÀSôþ¹?ŸËl×F?¨™1ä°l?®.t——D?¸¾¿Pñ?ë¾5ê¿ôD?¥Óñò/¹ª?ª{zô¸°'?•òRŠ"Ù?´Ð"/6O?žóܓ潔?åmtWÑß?±_´ÏÃ!?±×ýå?¥¤q4±É¢?ÐÞ§"Շ?°O>V9ãö?ï~Øù‰vê?¤'‡¼ìØ?€¶êº?£úAnó_?€G¼ìªÄ¬?*a$›»?ïâݧ²Ù?©V˜/d±?†7.«¿*?'¿Ä1ºæ…?"hø™«Î?¢iã‰\H?îª8ù¤NÝ?|	±q·?"" ¢¦¢Z?€åã}þ‡?—$À(ς	?"'³íã?ì"Ô¡?—Û.åE¿}?¡Q€ÖH.j?ˆ}¢ÜÓ?¶@Ÿ€A—?"ïR§¥rAGN3FGL J0440.8+2751@e'@¿ã°À(h> Ìÿ"À9È£¥¦îÀ;oW6Gºª¿Í
à6i§@2ƒÄ›%
?ÿ0/}HÖ¿Þ^ëì*h½¿é
M`äyð¿Å³Ï¿Š2ã¿á±¾™XV-AGNbll?ïóAc!¸b?R2E©­ºð?)50ü8ˆW?$xfÿ̈́õ?VV"&2,Å?Q+ÁWÙDÒ?ïû"xÓ¯?žM`c –ì?x†]j|ë?x¬ÇøhcA?–~ønùb?›év\Å×?îØYۓ?‡Ô7WãŸU?‡Úúž'"?r<íÎ"1?™G5ãU"?'ñMˆ'–á?íÝ1‰dî?žŒÏMF	?T¼ŸRøÍ?W÷H¢¹Yz?°Ã7ú¢†?žIÂK&Š|?ïúaÝ•{?;醽Äê?w€²E?"'úâ¥?B¶¸g¶#?9Ož¾q?ï³t›!Gè?
]Ã&ö?bՅ
6?a€h¨…y¸?|ÚïûÕÒ?|³è_…c?ïŠúèLJÇ?lÚ#Ð|H=?w²*‡?^rWªC²s?hEÔ"à?cVI)ÀöÜ?ïp6ì¦1?x1šê˜ö?QN±¥gK?Aù͝å¡X?è݅žéN?wO´î"¬ÕAGN3FGL J0442.6-0017@h¦€Ÿb0wÀ<vŽ ¿"(À7±åvø…À;EŒ^G³ô?çÒ4oý@»O)@÷Íÿ§Ày¿äê/ô^'¿çÜ+0ý›¿æÃÔ;è¿ë›‹¤•¡AGNfsrq?ïõ«ezÞ?K®bùG•ë?GãyõóNÀ?E[kX¯×?Anðð÷j¿?8|î}/=?ï—Ìë*°Ù?‡	Û-à#q?fþíU3[H?sEû6í}?"M	îXñ?>"GL§?î	`Ǟ˜:?é+²sJÉ?œŸèé
M?'çñãªf?¡ÿ
DiÅ?"§çBÍb§?ïÝ6Ïu…?t›aÉâJW?*®>*ˆ ?= †v`è?p&c
5?tCvЫyw?ïù¯ðYU?@/oöH¼¹?>D®7Ì^Ê?7¡]CŸÈ?4;Ï`§Ý?)ëX¡mÆ?ï×	 ¬w1?mÿÀç|«–?TŸ/¯"Þl?Sƒá5Œ?n¦Ç\?g'«a·½?înoR"mt?™úCF‰xÐ?˜V›¤(^?'ò™NÀäS?™ÛzJ;,?"G÷j¤z?ïù9ÍV4•?YNi}C¸í?²¸"Ðû?Ò³¨Ç.?I]Ÿš_a³?YÒVm/AGN3FGL J0444.5+3425@dþÊ€àÀyU E…EÀ9æoD[y£À;O®²0?à3-;Cð<@¦|«ø@wÈ_ÂX¿ Ôrªä¼û¿áýò?¼È¿åQeà7@¿ê½ZÅÑäAGNbcu?켄yI9?´58 IOï?¶ŠßÞ]ª?³tƨ?Œˆ«PÅ"?…<fötµ
?èþ7€]1?ÉÙ¥‰xˆ?©"0‰‡>'?ªË Âp¼ü?ŦÜhÔ³?œê½‡¬?ê
kiõ*ÿ?­-%6"ò?ÀxM $¯?¨|–#µ•?­HဤZ?–'AH"/?çöü½¨U?¨Ò<÷:?¯|»È…¤Ì?•×‰)º§?ÈDÞ@â¸?¥‹ºØµa—?îþ‰:{ÑÞ?¢û-²e¤g?š^ÀZ÷?¡¤ün
_?v}çµO
t?t]óåPJ?í‰Ee(½?¶49ü­é?"&Ûçmè?–²8öw'?­ZþÍr1?±…E+ôž¥?íYýÅƦÌ?¡¬…Ä‹(?¯"aò?žWûV_ú?•š>… æª?"SCM+^?ìÉÔ y|?'ŠýfËû'?¡"Lm_â? wæ^ÍÐ?°ç8È[Ü?Ž>Eþ'AGN3FGL J0444.6-6012@pàŒ€AÀCs`ûH
À:\f('ðÀ;ïë‹Ô´ù¿òaohی@^©WQËz?ÿ™¾×ü¿î#ߜ]?Áh%£8æ¿à•€œêÔA¿Ö7‹~ñ*AGNfsrq?ïõ³º›áŒ?Qld%;T?'ÕíÐ4ãx? !ð{ŒÃ?QÍOIJ?PœÏD#ƒ?ï'Üd¼º?ˆ)·Bþ«?fdìùpúS?qý#ªE¸˜?‰ä͝ÍÈÛ?ƒìô3:ä?îøÿø•ŸÜ?"=†"˜{Ê?†³"|Q	]?q7•Þ› Ã?•†>¦ŒyÔ?~'œ=Šà?ï½®cL£?v—Y¾ÜJù?8ÓÈiJ_?<'"qt¥§?ßu?vkn•ŒR4?ïú˜/"˲?7í~t¥"£?ļ¸?Ä	¸s.?B=¿*ɀ?5¸¶XÁ¥?ïÙãð™Ÿh?kU>¶Í»?R_ôÿ"@?PãU"wìÚ?lìõµ@@?ewŸ?ì>?ï"÷M:,?q¿Å·QŠ?y£7_8H?gÔý6cÌ©?'&¦pä7?h…£ic]S?ïóŸ øð?O¹ϐ?×NP-Qü?"d3(?W£IÀÆ2Å?N¤LóVÁAGN3FGL J0447.8-2119@kŽ± ‹ü"ÀB!ÕߛªÀ:Q˜y*À;ÉlËu±?ÄhÔÏ>…æ@GrÄm­­@`¡ ¤$ã¿äY@í ¿ç֗4u¹§¿åÍ‹gb÷¿ïÿ{j£ýAGNfsrq?ï¦<Òeµ^?…ûŸß^é?NÓÆýŽî?JÈ}¤y°ô?"ƒŽçÐ8†?…4^§6Wƒ?ì?4.
?´7°óâÂ+?¤þCŸ3ƒÝ?¤5зâÎ?³‡<¿î›?®l'E.ª°?ìígàA§H?žV©Gq?§é0Plä?tdõ°ÃB?ª˜ÍLì›?•ð²r=?é°õš(p?¬ð½¡È?²íU(Ê{C?¡B¡ÀM›;?¿ŠþFMº?¦…òCÝ?ïޚQûJd?q,z­&[?CÃT=\VÜ?=f'Ô.8?ltØÿfü.?p;ç7ã@_?î͑G²én?™Öe&ö9?«s'2g?Š/GG?—x'x¾ù?'èêûç?ît¾-w²i?Œ_õR	ߓ?›»Æºðôx?€çь¯cK?•¬sœ÷ö[?€¾Òu®?îA¬ñmI?ÐLZ·á¢?˜ëÑ;%Ù?"Ò"Iïn?žÞð-'•?ˆÅÚÔÈ$åAGN3FGL J0448.6-1632@jà»ÿŠ;ÀA6¿Ý/ñÀ9AÞíwÀ;\ä
[2V¿àÉ`í¼Â¥@'_?ý¶¤^ïy ¿ÅÜpGª¿Ýˆ_ãý4¿Õ»Ö[åÚ¿àXU¨9UÈAGNbll?ïðêÇŸ?R{n‹Müb?@ósq"…?:¨÷}>?U°· Û+?Mf^†ƒŸU?ïm`"`]Ÿ?Àí¥ÈAœ?k>þû£H?g¨ZÃk2R?Ø(sÃo?‹|.%Œ"?îé›-S±i?ˆ™.*äÔ?ŽZHUA@‹?€Gÿ¾©­ë?"Ÿv)1d—?€ksžaÅ7?íûqb:T1?"Ø!Ù]m³?RͯQºþ[?P2;kÁvÁ?¯²|^]Hÿ?"ª¼ÿÅ9?ï÷Ôúæ(?A¾sŠon¥?6ó렅?0ðYå S?EŸ"¬$¼?9¥}3êÿ?ïÎÒ¦U"²?r½MՀ7Ž?VÌ|@ï?Q®½X=ÁE?rãî¿Š ?p<‡
'?ïrÊvA‹ø?x&5ýE™?"Ù
ÂÊ6?p:ÙøàÎ ?'*‰Vƒï?p¹oTч?ïpMõ7¨?t˜4–?CgØQäµK?6b+4wÌq?'[™³%ú?sÅÖ»Çl•AGN3FGL J0449.0+1121@gm ìt2À4ª_ºz»À7䨮àR¼À;:ŠE–ã?ý€qÅ?9Ò@¾‡d¸¼@¼³Ž7eÈ¿âFWÔ8 ¿éU;)]Ê¿è[•'ïx–¿êÙèögêAGNfsrq?ïwx4D*Q?•n&–Ô¾?‹ËVXËJ?"ú×H½
[?i[f€¯L?iFDÓ.¾Â?}½p?¤Iÿ]°Äµ?‡åÔv2Ž?ˆZt‡"Î?ž}f­êý? ¥>ºç!V?ìÖúöUÝ,?§zm•!Ï?°ò¸9òÞè?¢o$î$tú? ªà%àˆm?™°ÉÞq?î"[šŽ?¥;ršAÙ@?"u`s@'?"h F	?£Õ6"ë?¡ÅR¦ˆBï?͕ìÞ?š^æ'U4?‡&š|?˜ÉJõU%?eQ'ÑÈ6?l-˜ÊÕ¼a?ïmϜ
H?`÷Z¢µb?x'
¾¸l­?uLk&‹MZ?ˆC'p˒?‰þ¤—é/?ìPþÂ0›?©>vÙ^A?³|Ó¾|ª?£§¸z·)˜?£÷ú:'Êó?šð_ƒ[/J?ïX¼M^é¬?Š
«¨ÿð?ˆ@êòJâ\?$¼•w–ÿ?­c¬Ì?Ú*>AGN3FGL J0449.4-4350@oΠwmÀCôäàõÀ6Ñd‰"—À:Léki¦?åÅ~Ä¢@Á]Z¤k?ý•\ ¿Ó•¿ÜFž†#¬>¿Ýs䧯޿؉k?$iR¿Ü+ƒÆAGNbll?ìɝ·q­?¹gêG?a7ø¹=Š?dξ·.ٞ?¹-‹L¦?¹/GÀ	?ïåª¶™Ò?ŽèǀçÚ?jÅï?H¡½´¿?‰у™;Ì?ƒþ6~M­?çIÙ£}{´?¶XJ CZ?œñø	ÏR1?–{–®•›?Ï:Zq ¨?µ¦²îÀ—©?ëÍjaGÎ?®ƒ¦ÝÓD?OQûÝaV?PΤøü5Z?À«Zlø?®xomðB?îs7+#?¬-JÝf%?T•õŸ"Ë?\DDfcÜ?¨,0"ÿMi?«íb:$Ÿ?ïÒʇù??rUP¦úíÕ?SÒí´_(ì?QϹSWÇ»?q¦"†T?oԎíV ?èü`º;5ò?²#'Nšå?›b?"ìAÒËMù?Èm©ªø€t?±)ɪ'í?î!@Í$¶n?–ÎVI>¶•?QrÕßÁÙ@?Fԝ—1`?­`\€òIW?–ď›ÑÈ®AGN3FGL J0453.2-2808@l¡i@5z5ÀB'HàC¢À8iüybÂmÀ;ŸüJhÙÞ?ôPBàÐ9ê@ÓÇ©¢PL@
€€mùƒ¿å`tԊ¨²¿èýhæÉM;¿éf¢®7­¹¿ìá£ÙŽ|/AGNfsrq?ïÕ¿HăÂ?m`òŒ6ž?h¥óÕßIï?fg¹ÖË?ašÃS¾üO?]Æ©…¿ƒù?î×ÖÉ$÷†? …ÙiÛi\?ƒy×{ˆ	?ŠJì×Ú?›H;MËõ=?˜})c‹¦?íøÂ!y?›ãaÂEgò?£§zÕI£?"IÕU"?™ÆmF±=›?c¸˜)°g?îF÷¶ý¥?¢v–ʲ@Z?")·¾°šá?ZÏAä?¡Š4¥7Ø@?Ÿmi¤??ïÜW±€?oyÐJ•%?h¼ÞV-ÒU?i?ҜÓ1?U×AW|«Z?VjªÿÙ¦?ïŒÊUp—9?''3a?røâÄή&?m£¹.êŒ?ƒPùJa֒?{@0¥Aöù?î|M/!šs?'ë{< ¤? {ö[¾?Œ"~:©°N?Cb,$^?ƒez`æ
?ïšx%Dvì?" &_¼Z?xÙEÿIf?kÕ«4K?yê¨F"ð|?€ÔÅ¢]¤AGN3FGL J0453.2+6321@bNO€Ü3r@(Y?µ!µÀ9v(ßóÀ;[‡æï?âEi™KÀô@'–E&@Æj?Žá/¿ç¨8_å:N¿ç⪬]ãØ¿Þ²~UNÅ¿ÛÀŠ0'flAGNbcu?ïéÏZ#jœ?fGYû²à?Iõ˜ÛÇÜ?Iªœ}/Œ?_fÁ-›êc?bÄä%ËÃ?îÍÄWn
?§èàäè¿ ?€éŒ?"	gÛý†?Ò¯
>ïä?¢ìë û?îχw5Ó?"« k	­?"?£da¿?va=Uu¦?›ïJø,?°5gjó>?î£åª`³–?"#ÊåŠì?q'fFkÉ?sSîboœ?£x{#?'—­‡í\«?ïñ7f=?E¯·")¾?9‰oËM<µ?:î$â"%Ï?W/"ŸRÒ?B}qþq¡?ï¬c¹ôê	?…²\fÔ?f™"ïàT?gÿ×À?~'png¾?'³¾Œ®×?ï™è÷zËM?z«Iv~?r$ .hZ?e\["m4?€s²ßQŒ?vÞjÝX0$?ﱆ!¢ñ?ob{Á0¨:?eaÀ͂¯¾?Tø
¡g?|Œ#{³"?k¬Œ	ÀøsAGN3FGL J0454.6-6825@qzw@=ݱÀAÚÁÀ)P[À9óLŸÀ;ª>"E]?욆 \p2@ðÑ›¯ô@"ä %\¿ãƒ"^ϙ¿äJRŸ	E#¿âB;¿┿ïÿ¸èz0OTHERpwn?í)iÛ»Ó?·)rO‰ÈD?¤±œÃ
Of?­'û¸ìœÖ?©Ë̜¦>n?¯·‹æáG™?ÖHƒHì¥R?ǚUæ*Z¶?Ú§
çZ}á?ɋ'ä&Ã?Πݟq¹›?½̘¹8µ?æ?\jþÀT?´¡AÖ$"~?Ê>ÁÔ¼?±«<>=¶?¹ÊŸ$aÍê?¡º 0xÎ?Ú4>Ç¢&Â?¸õ
¡¢/H?عjkX?¾€>‡WÖ?Ê$­˜mäN?°Èé$¶u?î·C¼s[?§.`6?"¯$Í7¨?›°B;²?•hyžÎøü?ž‰÷Gòn?ä‡_‡úà±?Ä £üž÷?ÎëØ£?ÁÃd'`°ß?½îŬ-V6?®*ý?ë)ÊÇÂu?¦¸Ç\Jƒ²?ºõZWí¢?¢*ð)ÚU2?§xžÓ8xw?'àJ–hV?åü'"»?®<'ì&.h?ÐuJ#('à?­@zãXÑê?µšö7'ª+?˜¿FNsFMIXED3FGL J0455.7-4617@o¼@ŽÉÀCi·?œÎÀ8Ÿ>õÀ;¡1$e:?ï.9Ķ˜@ßqBn=@^àAHË¿å^WµYÏ»¿èBs'‹ò׿çw'&Ç¿é¢AcÖßAGNfsrq?ïõ{Z6?H%\3· ?Cz²±X™?=[~êwi?F‡Œ¬Ò2??fà/ˆ'‹?îÚ­7ÂJ? ҕÚ4y?€¾E`Škî?=jZH—?œ^§¬âº?›s¿—ŒÑ?îðº4;=e?‡|Ԛ%X?ŒmG€ä?z4€)ùÖ?"©îüá?€áI¹¸ð
?íݓ4n£?¥'"X\?"¯x¹Œ?‹SiÕã?§Ï°èšÓ?£J2¡?ïúᏞæW?4¥ÑèÔr¡?5ªëæÂf?)'ÖLόb?3H–Yîo§?(%gKöD?'ó)z?†Øȏ˜'G?r'È}Ïçô?k—ÄŸÝ œ?…Ž·=nu?ƒ`¼KQå^?ïk¤Ÿ×?wšqnñÿ?ŸtÓPDr?ip¢ZU‡?ƒwcpáD?q=•t_e#?ï{ mïØÒ?‹v÷†že?|°N\D}?jç|WÊ?'ñc
õP?‡ò؁	JšAGN3FGL J0456.3+2702@eì&?šIÃÀ$ÔHµ{À8෋òçêÀ;-hÁŠyk?ñYžqŕ @Q¸Ð¢@®i t)¿àʵ4D¿èAÐ…h¿åP‹¿¼C¿ì8ÒXõ1AGNbcu?ï-§Œ»(¤?"Qþb?‰ ïý"?‡:µK/\?Šõ,Ó¢ÈÐ?ˆëÂi2×?è"qm;ÓÒ?É=pÏ¥?­`HÒó%©?®+£x‰Œ?ÆZ(ÁÚÎ?ÄɖN-?ìÞôö?¤·TÁÉ?®Å&Ñ.È?›Ÿèuò5í?©Jkö'¡ö?—Å?õgâ?é'Ѽ[÷‰?¬rÿL·ú¿?¯h)@2x?žEg*kt?Æ®¿_j¸?©¸ÉfA?ï¼h"u˜*?wç"HÛߺ?tĄVIäT?pø¼$Å?jÔ¥zu¬?eD;S:®?솊PÙêË?½v"Q£X,?Ÿk80ùö?žð–\v™'?³ðßx6wª?¸ÎI{Sp?îpPbC*?"ü_¸Z!?žráøAÀ?‹ƒú³ÖTã?"h€Õ¤øø?"dÈN\]:?í$JOY"?"¨NmjI?¥¿Ä+·•?‡°I²œ7?§û–âû¥b?'hSMj-AGN3FGL J0456.3-3131@m+VŸIÀB½¿é{À9ΈJ¼½À;æHEéï?áX쒇N
@㹯c°T@MbÀi'¿ã
ºægÊâ¿ç©¿ê;Gª¿è1Nˆ	Š¿ïÿãï—ìµAGNfsrq?ïðz'¹?b´m¼»B?#ß¿ŒÆÒ?"׬1ä§l?\¹cëå$?a¼Ã+l¢?îU…Í"ÌÍ?¢¥©°?Œ->f=Û?‹~fµ¢¬?£œS"h´?Þ}ö¼9¡?îâøÕ?9?ˆv/tFTÌ?'"îž~'?}KM,ïÒT?'ŠQoaÌI?PlžH³Ù?í¨´n?¢]JéQ?ŸBÉè{[?7—äIõ?¥Ýã6Ðßr?œM醰¢Ž?ï÷ó{&*Ñ?P—ðæU&?'¶¥½Ið?çòÆÂn?LM"v ß?PÓÌááÒ?ï\ÆË3£#?ˆ°Í+±"'?z᳑Ïå?rÓÍ¢?‹]sY±$º?ƒ¸XŸÉ÷j?ïOžºQg?yFFå°\?‰Ss?o¸Ö4"q?ƒJ$QÉ?qbã@«èŽ?ïs+žòÒy?€Ë"ߛ4
?'ƒþS4áÛ?k»«µ£ú?€±"Ÿê?zͤk¸=|AGN3FGL J0457.0-2324@kö©Ÿ¡—ÀAr–¿Ê…ËÀ6uQ'ÑÀ:£º¤¬S@–íw'2È@ Ïryð@à"@¿7ä¿ÞÎmЁҿäQÍ_™Ã‹¿å–À™¿éxŽûAGNFSRQ?ïKn#°E?‡<ÄC Æ?x[ÉàúM?|ì–[>œ ?y=íEC#<?ï1O:?ï'bI1ˆt?…WÜ"Ïz?dêÈI©?f¤ó=œ' ?†,»«ÚgT?'28™qÿ?èÚa"íK?³n&å©?¾ÈOz½=?«—0¹ª\ë?ºd§ÁÇØi?¨3ì:­#Z?ïðhžW¢?mýxÊ4v?"i§ÓÂG?>IÝh:â?]•ŒHí?mqˆ7H§?ﬨòÌ!?­>úkà[œ?r&ví¼8?'º=$¹øÔ?w…~‹k6?¥+¼sóžœ?ïÜCrpŠØ?k=OK)ºˆ?Qö…
¤?Q"`Š¡ß"?jÁE`V‰Ô?dOÔº&²?é<?'w-?±£áÃÕ<?Àˆý	€‡O?¬"ÃæÀ?µ³l©w?¥.§$ ?ïýcü©´?H¤hJð>þdt<ˊ?i@îLî?5ÚùϪÈ?G咳ë%«AGN3FGL J0457.0+0643@hDàÚ ËÀ5°cÀ™¸£À9ämBùyÔÀ;r#QA;¿ÿzr·Ø@ÎÆQ@a:ÿZh¬¿é ?Ðû[¿ãu&ǃÑu¿ìù×bä¿¶õÅÿÔ0AGNfsrq?ïÈ÷Þ'?zžæ?Nœ?iP&èÝޝ?qñÿt‡kæ?m·û$;-/?n<ê Ý«?ï—òaÔ'×?'¤\‹Óë?gpoÓDY¥?imÓ{ëC?"'K™"¼?€)î.PP?íÿǫ̃î)?–¦c"¤ë?˜;íÁäçK?…âZgO{†?£â¬T~©Ì?'f±¸òÁ?ï–GáQOd?"Ìr;ç?
—J-®=b?ñJôPÝ©?ŠSp`'l‡?"ÁŽPh•?ïçù¸í?oÎy"#_—?TY@Òæ?`°z'­Î?]ó³Å*ž:?brJW"ò?ï×a´ø?lšZÐÙ;c?TôÄ`ã1Î?QóÎ;ˆQ~?n$'ضP?fXÑM¡?ï7zþ44?ƒC#Jò¿h?†óo»ß«?wä·òšð?‹HñvÕh`?yý:/&5U?ïë¸(±?X¥0X9áN>Ô;m‰>ÕN$jPUî?d=ºY…gë?X ‹ŠgŒAGN3FGL J0500.3+5237@ctÙ_í¦a@e©ÿî7VÀ9h ƒ-FŠÀ;]€
|ZÄ¿Ó`…'F§ë@
[¿Pã@Ë àJX¿âæ=@¿ëD8>4îõ¿Ýa'Èýµ¿Ø—ÁREG2OTHERspp?îÙàÊ8P‡? à(êÇîó?nÐ#ö¥´?nŽQÃ5Ü? tñ!H'®?Ÿ;æ݅†Ü?î^7Cõ3"?³ý—&ïûH?"y3Dp?"$Cp+?¥mzÉù?±Èà…Xe?ì{hÐ}?¤ú÷BOù?¡OWÄ÷'(?ŒÛÕ@s>?³}ƒUå"? »:¼ Î?ìžãñ_0ñ? ì|³i=?r%ÊäC!Å?qʔøÅÛ?¹æƒÆãBŸ? Ä\qã´?ïɖ*4˜?~fATímÛ?S¸É_Wòç?Uòõ[©Ï?vF¸­z[ð?z©%I+ë0?ï~ûržûP?"NêºA±†?m"ñÁ{Cn?qNlh>Èà?ˆÜ&ïÉu+?ÝŽÞL‡?îñÝÚÞÊ?…D†zŽ[?Š,Yw?t_eòù?"®>ü›ð­?~J0Õæ÷?ï"ˆ5n ð?1`s}é?`îÂ
?N"‹4d«?™®['
µ?€Þ՟–uAGN3FGL J0501.2-0157@i.
á'6À9E  œWºÀ81dÒèoÁÀ;Zl ºŠ«?óÿ2ªøÈ@³¬wâÆ@OB?ë}g¿ã÷|k¿ä¿æ@àùˆ¿å¥\jÓ¿éñ•S0KAGNfsrq?ïî{VÉ¡…?]Ôê§Ïúk?S‹èA÷·?Yݯ©?NüUí:µ?G2qT?ï|"lÅ?'H$'ùšË?ln²aÒÝý?n(5KaãU?‰ÛÓVÒë7?üŠg"X?îäÊû™òc?eºˆ2±?¶5+'ñ]?ƒ'èúRá?'°ka/ÂQ?"ġ㝧N?ï¶uŠ›¤â?"}ñ"ϧÀ?O¹§¡%i"?VˆÝC?€géJy#?ƒ£>òеÄ?ïö'ó\P?H_D(k¾N?Gֆ"i?A´·ÅÕ?<;Y¶Óîf?3ø"!s¶?ïË ­4++?tA+/äã?\·/Ôqmi?Y'¸–½?sÝZЏ\?pCöNLP}?ïLFŽž'¦?žÿ8Ÿ£³?ˆ7÷]Ýl?{´±@Û?"¶dýñâû?tËÀš{Í?ïð¤sÎj?b2"›Þ¾?=3¼`êÆ?B°ñ*»?Wj)š¨?S?`™ëê}VAGN3FGL J0501.8+3046@e¤(?NÊhÀ5pÿÇuöÀ9Íøí½]À;WQ§'€¡¿ÈW%«¶&Ã@ÃɃl0«@þÿÝp^¿Öfm†¯ö¿éíq—
â̿췋aiô³?æÉǓkÆçAGNbcu?ïH4½…z?—£¯>"Ûâ?w8Švk5;?€¢Óˆ?'+E±˜œw?"Mì>y"É?íß'?+†c?¾Y'I¾1v?'>°ÜŒ¡?‹<&O^²Ê?­~_,­ª?¼˜Íèfí[?ìëcA݉Í? %ärHL?¥''Yù	…?•
µ)†ÐÙ?¬"9‰
@¦?–ôùÝJ?ï&ëóiÕÃ?žíõp?*Ÿ€6vd=?BØ@Èím?šíB'‰¥'?žñ€'4ì?ïÈgGŒÜr?zÂoە÷}?X@¾Ã±?^Óx¥?u¼,"ÌC?wÌj'z?ïcs]ÖÜ?¡(vóz¬1?mí±¹ííD?u昇ïÏ?§¼Ö¦œ?ž+òp:õ?î®Òc9¶/?'ü¸{EÁa?"ðùtB˜?ˆ¾øÄd'è?•4º$‡&ƒ?ˆh%¬'˜?ïá•éƒ3H?p¢Í]3p?œ6$…ƒ?i%KtÛà?n¦v_{?p(šf'ÃAGN3FGL J0502.5+0612@h>ìß&k¥À4Ó>¿XpÀ9ƒÂl º‹À;'ÅPÉ?¬î"É€[@µž´5§,@¥¹ß_K•¿áS¯¸пì4k‹>b¿áÁÄ|àë¿ïúÕ	öè™AGNfsrq?›íJµ?£"¬Îæ¾¢?{coKa-?_¸"Ùû?¡(R²…?¡³q³«Ñp?ì®6N›™y?¶ôØÁ ?¡Þe¾…=??ž:¦õÏ?±Ÿª–»?³ )"±?éxM+ãð?¬A­|(O?·KÒóI¼¡? zè3ȓß?¼ñïË<Ý?¤ÈØîº?ä"ûE8ÌÙ?¶)u'žñ?¨2uÃ݂?™…¾C½²?ÓÕ#&ºm¾?¶6¨ÛòRÅ?ïeñ™j[?Ž[ZÿE?pK÷á^»]?q!%ê^@?Ž]½¨ö"?‰ õÌ5Ó?îǪ]®~P?¢Ñ£_æÑx?Žàº¤Ýî©?Ž-*%Z'?—šVû0Ú¶?›ßeŒ¾î'?ìÓ%'ƇR? ]ú¤Né?©†¦K#õ?"å,m…å>?©G8tè?•·3eš?ë8óðé?¢SÂãL8?¡Ì»Qq¯?†ÉñÖ:—}?¿µÅ3Ñ=Ë? ²)¼–AGN3FGL J0502.7+3438@eD¼@ŽÉÀ:ƒ?»òÀ93u@ô¼ÖÀ;=KË°m?ìN–ž×@èÆUå9Ö@JL`€É>¿áÿVÛ6¥Œ¿àKTš¿'¿è:¼¢ï>ù¿äû¹*>ÔAGNbcu?ïÎäǕUg?póu5Ç?k=$Q,¾0?iyµç@¶?eÞ$|š†?`;Kætr?é¯cCW~Ó?ʌGíª?›žuÖ®¾h?¡ê˄['?ÅΤ9e?ÇûíZПÚ?íâ.QˆD?˜hx²‰?žSŸ™[Ä?ñ¡……ÂK?¢³KbÓ) ?‰™ù>õ?îÈßz×ë?"†º]@?xs=â&6ß?vQÞlKö€? c š\µ?'L,½õ°?ïíñµaÌ?VÇl)·ú?Rª·"êY[?LZ$Ú
Hÿ?QsE0YŽ»?I¦#'ôß?î$
؉Ö?¹£ýêü?…4AÃ?pý¸	î­?¨rù—ˆ?¶4Éìͽ?ï(÷´Ns?†Ï5Ð.r?ŠZ:ó–Ç?{õ¬k±²?‹ž"Å8?}$õ¬	ËÀ?ï§P#Xõ?ut­*Šã?g÷%O_?V«`ª§?€.â֑?sw«è¦¬AGN3FGL J0503.4+4522@d7  ôØ@¯rú6<À98‹ò)ôÀ;3>iȶ?jÐì1»@˹ÕÁ@á€.¹|¿ÚÁFíá¿íqÑcµ\¿¹õ¯ÞÄ4è¿áO.+AGNbcu?ïç'¿À'?p"å–ÅnR?2DùÜ°Å?9oØ·]?f®*˜¹?pݻҗ?á¤1—@'±?Õ¥·U}q+? ÜYgèV? saû·_Â?ڜ¤ÔFz?Ôhâpç¸z?ìÄbi›hë?£ÜS",?"È/{¦?‡Œ"Ú__÷?´ªàÕ›z?¢ Û8g¨ð?íòQÔç? qðÖhî0?Od¤g!{?S6'r\{?°/@ŽªA ? Qyɉe3?ïñŸÆô	–?eeqeP?0Å~q™y$?15H‹—"o?X6ÎE5?dßW:7Ø?èî¦tQL?ҁïǦ?™¼âï¢0? ÿi}Ù/î?É
å"9¥‹?Ð<H•Åúv?îŸþ2Óð`?–º…ó*¡Ã?€ðÁ
"7è?x*Îv_ú?¡Ãì'SÉ?•H¥,Â"F?ï{VÍíW?{X¦Î£"?PbÈ=Æ0
?B4è§/?ósFh?z™ÐәþðAGN3FGL J0503.5+6538@b'Î ‰ãC@,Ñeaƒ¨—À:X4õ«hÀ;ÇPܑeî?Äà5Á¿å@.ûJ¹@®h@0FÅ¿éqÏÔÐ7¢¿Úü›Ö׿ì[
'ÁË?Ù£@'ªAGNbll?³Ý3?‰Îå­x²?uµ3j?}QÛ|)|"?{qPv!\?€cʯ?ïUÖ7üèì?™=|OkT
?t(^ÇJQ¿?u¯
´'¸?;!VKm?•È5Æí?íÔþ1ý0Ë?›-äs?ûôòI¢Ð?GFýž?£²"dtlæ?''oQ3´?ï}ÜçC'ô?ŒÐÅï|¿?WÙ*ÿ_'¢?nîƒO¡š? Ài?ŠÝ°'¿?ïÏ_ËäçÃ?¦(Ÿ¹÷¼?Wok')?dCÊFíõ›?rˆ¾]þÍÎ?¦†úi>è0?ïÌÉÕ].?|œ¼͔?]0	…T[)?\á
°SãŒ?rOpAºÂ*?x$¹sÚ½X?ï—3™ú?NP`G?Ž3F\
z›?'mÁœ;Ž7?³{ÉÎ5p?ƒR#?ïï7'uû?a×ÚºQo?0$x'ö¹?;+Ò'¿á|?]‡¿¬œ¹[?a*¶H77‹AGN3FGL J0505.3+0459@ho0_®¼AÀ4ÜW?öÀ86ÈqyŽÀ:ô÷eýŠÛ?ûaܶ#é@ób–x'@Ïï=*¿á½Ë"Ú¿æ@*†!¨Ø¿éT‰;Ÿá¿è?nO"æýAGNfsrq?ïÞÔ§È
?kS"d~É?Ocm'þE?L±Ck=k?ig€mu?gKi¡ãvÔ?ï~n+¹?‰	ÅäkÉ?oÔ(RXä/?oÿóW‰é?ˆ…Zp¯'Ÿ?…´òPïû‰?î'|š¦—?ž0™‰Uß?šÇs‹Vω?"VðQ·,Ò? $|•Š'×?"ªÇ>mxÿ?ï˜ãKòÐJ?ŠÆVæ숪?NWÅìÓª´?]ø)æ?‡á°—^—??ŠO@áÅÎ?ïïQ5ìe?lnh®Œ:?Oˆ²·ÈÇ?jr'¾v¤ø?R#û	8Ÿ?I'¨"hòB?ïÏ8õ|­?t;ÔP©'œ?Zaù|¨§?X"U{Vÿ?qÞlá‹X?p+öâJ¼€?î‹r‡öž?˜1^[zÜ?š{"Ï2-?'è._áRp?""Ì(z,?Ž¬€¿ª ?ïç‡|ûB?k7¹í—?D€ÉÓððÕ?Aå'~9f'?cXP}3Åõ?j!"ð%Ž"AGN3FGL J0505.3-0422@iŠsÿ¬*À9…Üßi‡ƒÀ9Лx–ê"À;pæDm[?ó[
/')@
֕Î]ñx@
ú`-è¿ÚeÙµàÄs¿ä˾mA*¿çÏé°Äi¸¿ê™¸õˆAGNfsrq?Â:¹S7?½"óÂHÔ?䯜ŽCë?ÇaÔÂuÂ
?Ë;yŒÍ?Âùµãý?äí3°Â¼?̜Ëó^?Ê[J^H	Ú?ÅÑ2å'?Å]Õ¬²?ÀO}3åé1?àìäLú?¶D@im%?Ôr?µzª¨ŽÎ?ÅÂ_"FÉ5?©$7"ˆC?Ö…í.0?µ×ª»ôÆ
?Ø6É?½¥Qø_?Ñ®ùåV'÷?´×X_ö1?ØûåõÎßÞ?Ê!ʾ]Pò?ÛÈyjhîE?ÉÝNk.2?ÆwA=j¢>?Ä	˜¶€ì5?êû‹<Å¿N?ÂßïX+Õ?¶âíwF›?¸þÇD?²Ã*¢ðú?³Ÿãàý•É?è¢v¡`Ò?­.áõ?Ù:"ð?§J"_U
?³¹Õö?'?œoŊ¹,?âN;U|Å_?°
4žÀ¯?ÓQðØÅ©m?°F¹Kž`"?À#0ø—«? ,†nÀ½MIXED3FGL J0505.5+0416@h…Ÿj"óÀ54"Ÿ^ÕxÀ9Џº–iÀ;vVO—íÈ?ÒG»_ç5@<OM:?þ}q +Y?ÝÕ«:"]¿Ñõ¿èÁS¿¦FöLпäHMÌ#1AGNbll?ïžb*0n÷?ƒñBKù®z?` ëþ¯]§?^t&›/Ô?"?:wPµ?þҍ¾àt?íRø¤'M]?´È_H"?œóË;5?š¤ãœ"Ó?¬VæUYÚ¯?±ObQ¤zƒ?íÅhñA\}?škö
Üä&?–4Eî&Õ?…ØޔO¡·?¨MöD?"ŠË褮F?韱cdÔ@?±¹%5è›ë?Ió¶gýã?šë¸0™·?Å×ûûŸ¯D?±t5¥áù?ïØü) |&?nmå»^þ?JzÜÁI?HY,ސË?p2šu`L?kÖõ´T?îëšÈ˜µ™?¢ßLª"˜?‡¡ô…C8s?ƒÒ÷0èœ?–»¬±&è?žpÄÝ@í™?ï2ôpÍ?€÷,@«Žà?ƒ"ÀÙ"íR?pŽS2®_?çº`yív?yT·*r?íƒÅ•S—_?™é·^¹?–³†Í¤&?'k´Ø(9?¬iãDC·÷?•,GòâÿøAGN3FGL J0505.5-1558@k&€IRÀ>uàè@À:7œÓ	ý°À;͵±þm¿àšŽX•9Û@
2"¤Åœ­@ÐúÀP»¿×'ƒk7¿ábvs5¿ç •—‰ýx¿Ð[±e¬ñÕAGNbcu?ïqI›vàÔ?m1b¡Öl?d³wØPþé?eIª
8#?Ž€»"ì™:?³*ÔxG?ïQ€‰ðY?—î`ܓÞ'?sÓì'dG"?‡Ì:GMî?Û…ñe?"@ÃSL9?íŸ?¢úÈ?šX6ĕ? Ôî
]r?_ÍgsÎü?¥ø0ÞC?Ÿ,Ø/"^?îh?.
¡¼?šÓòŲ…?eX{À`p?i;No*®u?¨+皛†¶?š4W"B?ïߗQ2Ð?o'ñ¸Ç¸¸?DÊ8º[?I¼Á"c"½?k6 +«¡?l'ú:8¡?ïÍR:#V5?tú!$+3?ZaÓÊa÷c?Uïß+èE?r¾n«cƒ?q·B0'ýì?ï¯ Çÿ;?…/À$,a?Gå‰ì"K?€Ï2b¿Ç
?ÌRGƒHá?s5öªq"?ï¶Å L*?pê¤Ða³K?A·h³øK?8úûÍg¢C?5ŸlU_?pe$‹i0AGN3FGL J0505.9+6114@b¢¸¾øγ@(0¶â—À:òÿf}À; ºö
´¿ñçêc5¯@(
e‰œ¡@;À n ?ìŠb=(¿é¬l'zk¿¸'eŠzº¿å5¯CéAGNbll?ïì¾s3‡?jP5¦M?+O>[G?*EþBödO?a~z²`?is,µ"0¶?îÝ¹V?°ûB~Þ5?zlˆyî¦å?yÐÏÈÎ
0?¢â"TM;?°Q®]?î³Æ.U±k?"òºì&cª?""®¾±æs?vò_gö\´?Ÿ=bÔ9i?'îVa´?îÖ¨ª¼?˜ìÁÀÇ^c?>™©± `v?G×`ä®?¢XK{Á{è?˜ÁÉçÔµÛ?ïúÌpA©?K
N"*?Âkzc?dÑ­C?A•ñ~ÉÜ?ISÆ5F€û?ï¨Z¯®?‹ëhQÁç?d"ÐFP?coàÛF?€Ä`"•?ˆkæù‹×?ïyï²ç?~`Í	"!?w\Ü1B?d«uöç|u?…í–$¶?y±ý&¨~˜?ïÁÒÂÉØ?pûö~ «?(ÂɹÕù?#€…¬g?~¬˜¡º`ø?pÒiÖ\AGN3FGL J0506.9-5435@pf¸À>-ÀBbë@UZ¥À9n?"zM¤À;P9Ø?çÅ
uÀf@ð»"k1?ù¥Ã P­m¿î[þ÷tô§?ÇÁXXg?²W\PT¿ØÞR—bÄAGNbcu?ïÈT,ŽX?{ 	ñׄr?Tl:¸¦
Ô?PŠtúßñ?vºÛ/Qq?xÃ;2–å9?ï"ŒÊ±È?•qwQ"?x"©~Þ<??tÍϏîV?—NDv(í?"nÍÆ¥t?î9d®3?—ŸÌA??"¶š²þ'm?ƒ;_®¼˜"?¤á\yu?'ê
Žc?ìÆìM#æ?¯Sù‡'û#?…LC´ç|?¹2oâ?·ˆÌ?®¤Z0Ñ?ïâ|ß%m?f׍7d?HOPÝ]?AÄãSâx?g
 Añi?dŸõ¶sÑ?ï¥Ü|±ñ?"r'l_?h¬Á™±Ð?eúö;h.?€]°}í[Û?K«rqþ?ï;÷tbŸÕ?ð|"ýð?ƒCz@Ÿk?q­býÞ?æßmoae?{ú˜Æ¸œ ?î Ä2kÚf?".
LJ¨%?‹}3fø?}ԓ"‹b?ž[:ëÇÌ?a$A¯¡AGN3FGL J0507.1-6102@pæ}ÀTïFÀBtߥíeÀ8ä(í_ŒÀ;ª3Ž¢Å'¿nyJè³=@ü^h–'@%ҟʋ)¿ç¬DScv¿¿åý '®¿çøbí¥¿éø^i¨÷AAGNfsrq?ïøõrw0?C©Ë ""?:G¾`'B?3v÷C¯›?@ÜJgð?9Úµ¤hñh?ïgߤYªÛ?‹& VN?my~ۓ¤?k"þjú­Ú?Ž©·k^U?‡¸x;ß‰?îâÿTÿ6?‰Ê'T4ˆé?Ž:|
þ¬?Qà32?"Øò—Yï?€q¨¥'[g?ïeЂ£¹?ŒÝ÷°ø?`H¨¥Œ>?aUú™Ÿßë?'<ÚÀš(O?‹ÊLÊ<?ïüË%'Æ?4ì1Júå?1i"½r^Å?/0Wüí>?,°%̌f?#ˆy
'm£?ïËÕö3?r-/±Sä?Zz͗;Ð?T׸Y<?svQ•œÓl?n	ûɒð-?ï€ú߸?€?vÿôC=ªK?dæhèp?qߚ¶!??€Ôé*ÃN?i;Cñœ
?ïä=5"`?fQ¶s÷uü?;¾n%Üj"?3rÚLãé?hJüÙªÕ?eÓâ9AGN3FGL J0508.0+6736@aùÖ`^åi@/È)?"j†À8CÕAæÀ:¿Œž"#¿Ï'Ÿã	Ð@lŠQýù–?ø]q?ˆV%¿¡âe+ÓÿἋw¤¿¿ÃlJÎQÕ¿ É^¶ÍAGNbll?ïòåŒ{Þ?azp2'Óu?'ýQÈå?"1ÞBïªz?WSŠË?afé?]†Ã?ïý¡UûŠ?•wPþ†;?rz¡N…?'`5.øî?†ÃFó Ìé?''f^¯¨?ìä÷ËS?§Qš5ý'1?"œ|Õ?Ž9`åA9'?³øžW•£?¥Št¢91l?íüœÑºûÈ?¡`´ï¸•?+‰Mhyc¤?6dP¤—«V?°
TÊò'?¡a{¤säÀ?ïø®³?OÊêa
ê?%%Äçô'?#­±3ñä?H¿¾ùJ+?L†hÚÃ&q?ïÖ¬±=>?|¶"µéŽ?ZS.	'|ž?RÆë˜Æ´?l)·ý9~Š?ztùåB'?íÂvHËd²?¢
Qêsö?'p³{ªáº?ŽËõÿy†ú?« A¸ãà? Cu‡¬â@?ïh´›—d?€IÎÄ3w?'rkÿ²3? m,Uó9Õ?'Îæ>èM?€•QÎaAGN3FGL J0508.2-1936@kŽ(`ܹªÀ?0Üà@GÀ:o4bÞªÀ;ð).ˆª?éK×V5
J@Uµ(Á?P@ÿ^@}¸?ÔdQ^þyS¿áòÆ7‡¿åGQ¯Z¿ïÿf`˜W`AGNbcu?íÏ4@0È?­¿hÔ2zY?¯gñ™ÿ©?­
4"å³V?}-uܶ†Þ?x×Þaº?ã%â‰â3?Æ1( ÛlÎ?ÌáØ s0,?Áä…üðJ?Ɔ="†?»ŽBïy?é¾:Ç7rÄ?©4}©+»x?Á¨
¿u:?¥ÂiçSç?­|Œ á×?"ÑÚr8ó?ã\íú??·§sžá–®?ÑñŸ$HØ?³Í½`é¼×?½R¢c£?©ƒa@)?ï1b¬%@	?˜÷®²,¾?•§
9w—}?—Ý	—¾Š?p²€õ£¥ ?joìTÝ?és"ì?¼ÀA'Çm?½ÕIэÚQ?³êb6"s??¶'žÍ…æQ?­'ù´°x?ìtÔ8S? êrdZú?´ñ×;U<?œÇ«G8p+?š*—G<§?…Ó=<v(?ëVޘ#í?£
$¬hÆk?¼÷Ѫ¤{A?}pXé·? ¢s!©«²?"ÖëØ­`AGN3FGL J0509.3+1012@gëý`éNäÀ1?Ê ¢¢WÀ9"Çë¼|À;Vj3z€Ð¿µÐF¦"C@#ȶ@zÎ]=s¿çÂR6ôe¿ç?lkQ÷¿æ3–òí•<¿æÎ8˜ÞïËAGNfsrq?ïð-Ŝ=?V§fÿòù?G]8¾Û?F¥%^%?Tõø€
?OŽþH?î«tcYe?©–\?þ?…ücjÿ?ˆ:ÈÓÃáí? :©Ôb3?¦/°o9—Ó?î©«dóÆ?bä«Íh?¥š€_»ñ?'ŠZÑП?š$ø߄O?‡HlÅ"?ì¨(	«Ç¼? +¥u•!?'i¤ç‡	ˆ?t㐅ä#?¸q‹"q?ŸË1õ¤?ïøh"Ë?E§Ü–,?7¶6Õ³§?4o¼YÌÉ?B'¥y~kÃ?>k×°…•?ïš+1ÜñÞ?¨$8þÖ?iÂÃ?gí,Ò:±Â?ƒCý‡¸?‰yø4F¾?°¦?^?v™}o5z³?zGö×<ÞG?l<w¢÷Wå?'/Ø]k?e?nê¢Ï»þ?ï!.Tì?€JÒ`ÞZÊ?i.@è 
?UÒq*>?˜¸2‹Dã?ù›.gAGN3FGL J0509.4+0541@hlë têŽÀ3 ¼€NnùÀ7YˆêíÀ:¬ß06)?תŠm+Òl@70BèÞ@Kù€_
ý¿Ü%<`¿š¿â¶‹AèÜ¿ÜNŠê ½¿â-ZfÜ`œAGNbll?ïç.‰šô?n+óqNéF?3Ž4/n?5º}ù'ÈÕ?fp"‡A²è?mÐ!k_?ï{Áv¤Äg?‹ÌÞqc:O?p>%¡òzÿ?vý1F±ƒ³?ˆð‰ED ?"¯°q¤?íËyÄ£CÎ?¢P£/ÀC?†»¿M!4È?VJC/'?­™sà˧÷?¡Ln8?ïQú.ëâ?'4fåO*?7‰-Ü~?EK –X$?œ¹Nœ™sò?'ØlX¼Ü?ïù?ýéG?Tæ~0%òa?&Ù¬CýÛÊ?>>
+ù?DD"v*‹?L—Ap–7?ï͸¥Mé?q'ƒGÔr?Y&®%ÓàN?Tƒ""ˆB
?rÚ£ƒ?l˜4+6'Å?îôë'x|?'ÝtNNf?~Þ:fºëj?y‡Ë+.!?™«R&¹?'^¦X¸¶'?ï½ÿý¦´_?qӛdŸ7Ð?,knycÇ?%µÿ­³E?€Rä3‡Ë?q·¹O¬õAGN3FGL J0509.7-0400@iæàé´À8gÀÌäJÀ: È{.tˆÀ;«'Ýãu†¿¼á'Ô'¬@
Æà#Á¦?úaäa\?å6y8Ñ¿à$«œ3ð¿–Ä`X™¿´žD—<OÅAGNbll?ïàøë[$¶?o»ÙAõ¢À?75v
°£?8¼2µ%Ç?l fŸ?o@Aœ'?ïawÀ'ù?"žéÒ¦‡g?rH¤Ýø?MƒS¤n?Ž~.ÁúÚÔ?=C˜¶9?î‡
FTù?jÒ¶Ãe?ÀÚ*wZ§?ƒ@¿s¬û?ž^ä-¢4?†¢"'??í²¹ì?¤¢šY"
A?V¥"¥;š?e¾/háàl?²£ «ò?¤‡Îq
ÛÛ?ïñTI6'?ZkZ¿…¼?)¤müÌÏ?(M",¦Ð}?Z"í•7·?XYחÃ	?ïÌ×ZU'?wHk[E.‰?YèÂ8ٗ4?UéÅŶFè?s"gGZ²?sÚOª2>?ï@OaÓï?ƒÓºïÙ?…äªá€é?ƒîPnò?Š|Ø
!?s@n|'?ïtà]€í?@®Ú1Ç?P!O"šR€?JŸÓã—?}¯a")?€þԞŠ¿–AGN3FGL J0509.7-6418@q$·@=ݱÀAš†@ €À: s,G‡À;ä"i·S¿¿Ú4ç
ï$ï@§E¥¦˜0@wœ'"¿éêþí¿ä¦¡H:¿â\:$áXB?µú''JVAGNbcu?ïõ˜Èä4ó?KÔ-ð')? Dà~‹Cf?ÐÂu¿­?RÅÒ{›({?Iü>Åé?ïó«ˆÚZ?Š¤ƒßFl¹?fâ5°ä(|?{§ü~ƒM?†Ê‡´Ps?ñÑ¢u9?ï&ôgÑG?'#Û4@:?'e‰"ºG?o]ûãÐe?'ÚÀXߺò?zrƒgj}»?mEd?'›‹Í??#\,î<Š?0èl6¦	e?‡	£»Þ?''b|m­?ïüE‹ØïN?0ϦœRä?#šÙþGþ?VÑæIwÙ?8''òX?.¿jè?ïÚ¨9y?jkXj±˜ú?R²jÐø8]?Pýê¤í–a?kþ'˜©¼ ?dlÚp¼½?–Í{7?h˜CqüÀ?rä«ÊÎaÏ?UÞž=j1?|ˈ¼–
¦?az˜[Û¶?ïóceÊ,?R¹%‡`ú?œkjõÚ?4ÒAÊ{?X|RÝÜ?R[µá:AGN3FGL J0510.0+1802@gû¿"ÿ&À)‡LàƒböÀ8ÀÂã>ÿÀ;7&ùz«?åMƒ2©v@øîÀ½të@F§ msK¿ä¿Ÿ±Fð'¿åîç²è[Z¿ál;ò–ØA¿ë—6Ã5ŸIAGNfsrq?ïäÅo"ê6?da–¦%ÀB?[‹XMçb?W© Ý6¥¤?ZéÈEÕ}p?XCSCvZÑ?îlôÝ?«*ý<?‹úIâÁ?ŒH݋òù?¢LÀó±°??§]~ˆ?îi#·Œ–?"¦ÿ,Bø?šG]÷í?‰åüï`gÍ?˜"+ê–@²?†Ñj$èÀê?ì'oOÝҝ?¢H@NŽSK?ú++Õ¼?ƒÑ¯W'Ü?·5úFu¦?¡ceQu?ïõON‹˜?Q²Â|Ó?HÈ&çù¸Ž?F
·—̇?AúžJÄÙE?BÁ´È8È?ïn:Fç‰Ö?'ï¡ú@ld?v%|øJh?q¶":‡øÌ?‰^ë)ç@?2ÝÏÞÕ?ïL;:h²?'|¹ž ®Î?ˆÙƒHÝ/?yAÀ'œe?"hםö́?uabUÀ'á?îç€"¹0?…4´á|A?ƒY{ÇK®?mj4') ?™Žc,5˜1?ƒ&÷Û*GüAGN3FGL J0512.2+2918@eõW´Àx=`2Å¥À9®§â1¸àÀ;9WÒNìÍ¿Ûb1ÍF^"@{——᳏@@¿ ¿â@^xõùÜ¿ã2»!1[ ¿ë"j2xοå~¶0u‹AGNbcu?ïLQ¾Iã_?"ü/—Æ{?‡;Riî×?˜"Úï°?…ÓU!üqY?'湟«Ñß?ë.Ø8'J?ÅÈÝmȟ/?–ßÓID•Ò?œªþ=T–¨?Àh¥I¿Ö^?Ã:^$q?í'1¥r:?™|6PV×?-Z3Û­C?‰ð­Òµ¯?¨F8–Æì¾?"X½"¥¸?í;èð*0;?¡"Úãò?y‰•>.?uwë>ç?´_æZí€? ÌÉ3šÌ?ïËêõµVí?týÙ:hŽŽ?e^uèú©Ï?cù"¸Ãþ?n¶"SïùE?pˆªû ·?îÌEIÏñ‰?¨I–'¦?|—õñãP?'¹¼¬õ")?ŸQY)?¤nó´µWO?ﶙ•Îð?‰.Ó-Aµ?ˆÛìqÐ]?}Q3]']õ?Û6›=JÉ?'ªhÔiÌ?ïB¥X-'^?ÆLY?Z8oÑ?KµdR'òà?–ÓâTnM?~e«¦B'£AGN3FGL J0512.9+4038@dѾÀ//˜?íJ =?ÚÀ9Œ$ôÀ;[a8)<9?è6âGæÒ@"WJê‰÷@͋?cÿäz±|íÄó¿ÖÔ»Ðóo¿âX[œ'¿ãäâ^É'ëAGNbcu?î«ÇŒ¤œ5?¥Þ÷Í¥'?ƒ^	ß©~?'x{K®´É? kßõdÒ?¤$¦CõBû?Çð'ùKä?ËëÌïî?´árüáb?ªú²ÅçT?ç£!‡†"û?ÌlTMEiR?ìlM;-?¡nL´š™!? V¹æB]?ßüy)?´r6'qã?êÉJ=9?ê}7cCœ7?¦
DÁ>é?¨óß3¢[ï?›{ä­p?¿œUK6	Q?¢ÑcÁbº?ï»j(+±ù?…ºˆ&ªŽ´?b9QŒòÞ?c×ÑpÊR?y.CòŽ?ƒs÷F^?ÔOé§%?Ôl%Àâfp?¶Y}ÓH¨?©€­Ú+J«?ã((Q)9?Ò÷§	!oo?î†?¤¨
?•ÝÓç:?Œ"
»î™?€Ç7þDL4? y¨–\Œ?','HsT?íÖ¢ý¬¤Ê?uï'ÁÛz?žåâú4Ö?géKp/?£"Þ§?Êp?†ÆèId~ÙMIXED3FGL J0514.4+5603@cBß72œ@$»ÁÎjÀ9|5Om&À;}Q›Ô}¿ë¼T2öç@œ,µj°x@·Ñ?Î!6¿è¡ø‹žþ¿éŸã*cÇ¿æƒxÒÇ-¿ãxÓ~ LšAGNfsrq	?ï´qì×YC?¢zP
%ë?E`S—?Q^+¦qÐ?†PB4?¢zñ¡ŽÈ?îm‰Hœ.¨?²&gíüm?}zUR`(Ã?˜L¦¹?¥x Çýƒo?±4ãz	ò¢?îˆó+ö?˜¶,®Q&?ŽXƒ¼ÇøÑ?~@+
|ļ?¦±^æÅg?•4FâD'?9Uó8?'÷N¾oŠÿ?Y5ˆélA|?U]z‰OöÁ?£½à$1Qv?'­#	%Š×?çœEù^{6?Ø­½L4?/zälÖ?A-ÍÜ–P?ÐÄÌOpÎ?دØÓÉÉÁ?ï–Où;H?â$?-?eQ‰"ÉÂH?kI-¾ž?…ŸN§gi?Žn'Ji‰?ï\Ï×̸³?ƒ«V¶•/×?yî·÷\Q<?j½(ê*é?‹Ô®bº{?oÖ,•ð?＀|H}?m,æóօ??6cäne¡?.ñ¬¥[L?€,ÁË4Ô?lzj¡«Ù/AGN3FGL J0515.3-4557@ow•@%NÀA¶ó=<¡À:(»ìª¸¦À;›ÕÎÔ
¿©åD²Ÿj@/ÑËdAô@p@.ï,¿éÝ"®Y¿Ö×c©ž¿ç±"£ï×σ3ÒAGNfsrq?í"öA»6L?°óI`ê?³ÛY"«?¯÷VêNf? ¨§_?o†*×?ì¯À¨[©?²]{ô3?¡U‡öøÓ? !͞ós?±öO$›äÏ?¬{ªfPÎ?èûnKjÀ?­Cê']ÿÈ?ÃeFÀa?©»
,šZ?±Zgjøee?š8(ؔÀ½?é B*Fûg?°Ð]O¤H˜?¸!§¸R?¬ÝWe<|?¾Üâ‹Su?§R«!V?í³
™ƒl?¯ŸˆŒz?°T§?¬Èºó :?'uœé 8?'©'z‰eœ?î듖8—?›×>jÉÍi?ŠÐß+?Š1'oó¼?•‰$θך?"'G}³ƒ&?ëåP§7g?¤¾Hg²Gº?ºßÌÕliÇ?¢Ð3|·¿'?¡bCÔ~
?É\S2Å	?íöÕL«²Ô?"0W¥r/?™kÚEe£?ˆ¿ôìxá?£ÃõK'»ä?ŒÑhå]¥AGN3FGL J0515.5-0123@iY,Ÿ/ېÀ5Þó_ތéÀ:™`sÞ.À;¸õ½†ß?èkÅd½^@
ch/>\?üÆ`Ìôe?Ôq'ð$b,?æ5ÓL rš¿ÐÙí­Ô¿äy¼*øÉAGNbcu?ïêªú{Aü?að1Ùݳ?J&(~›8¢?I'GìŒÎÓ?]–ö"{
£?[­¶ÕgA­?èa%_¦?Åtá†ö²W?½;Ͼ2™õ?¸ó
Ûä+‰?¿»VÐ5&?¼ºáùëÐ?î"«4>?ÌøS©Äa?JÔ(zŒR?U(Ž²}?Ÿ2Öowù?‰†¦·_3^?æÑ5]–n?ºeÏ°µrœ?É»‡ÞÊ?¹rgzû?¶$o?«þoӔÀ?ïõj3`»¾?OnM3R–Ø?4g<µ÷øç?3&ÊwQóe?PɌFkÇ?I¡Z!ªø?íaRܬúÜ?°sɚKë?£œ‡ÑZ/?¡?vðwñ?¦NJhh{?¦y #Jö?ïT}W'Š?|õtëA?½wÖ ?q!OÞH ?‰^ìÅF¸Ï?t÷êEÐ7?ì
m¥?¡ÂNEÞ1?¸	±3Þ?šËÅã`ù?ž²7×$ ?'²>.£|RAGN3FGL J0515.8+1526@gwÿ´€¦À*"ÚA)•ûÀ8Ϋäõ¸~À;.Àp÷Í¿ò±ÞÇ;@$M˜ö\@ŒÐ¿u¡B¿â׳Í2´¿ãtsè/(â¿àèÑÝz;¿Ùø1<ìxAGNbll?ïÀtõÓßÄ?yÇ¡[\m?Iï¥âAê,?C9Ë.ð?|‡gt¸ú?x˜îó™|?ïQ½jSò?™%÷[LÊ?r'þ§gÆä?sÇÂJ2–:?'#"Ãq÷?–íqæÙÞ?íÔ-‹d?›ß_:fòí?—,ªCùÑ?†Ç@®·\$?§&ÒO3=?•WB6OU$?î>
$^a¾?™_uÊ?P?>Góô¤
{?Anw9è
N?«âÍé~ö?™Gžß…Šd?ïî†Þ€ÿD?\d
¤åôW?<#ˆjVñ•?3Œ)wHˆ<?[é`ol"?YQßL¼Q?ïÆè¬HÀ0?y߬‰D'?[*}FBª®?W?ø(žAc?uÁ
>‰x?u~˜bÀ3?ï5Ö9ɪ?…ÙËÿ@"$?"¨Óz'C?vb3L£"?ŽjÈñ'#?Q
Fî?ï‰'k©Ç9?vd–0o:Ì?!@áW·>}?/¼>ZQ¶?q!Î'ë?v[Æ7ƑAGN3FGL J0516.3+7351@aSÊ€à@3Æ"à՘MÀ9ò¯ÑêBÿÀ;ÐùyÔt?òá']
9@‹³÷ñt?ÿu«€vÝØ¿åM¤éXôŽ¿èôA¸Sm¿ÍgrÓº°H¿ÖÊBÐpUAGNbll?ï"ó£êð?†p@4•À?l«kì˺e?kéåEñO.?ƒ˜<¿¸È?ƒ…Ì	dÍ?ïa@	½!?š3×?cåz?}šUþýˆ?{µ'ð>"Ç?ˆâÓ;ª9Ë?–:u±WÝT?ìfQ©H–Ð?¨1ÕÀÇ?«¼~o»?kSWR?­ÞàêsÎD?ž™dîÖ³?îˆ*"ܤ? i
23'!?"?çŠ2t?ÑìW'Ê.?¢o³qP&?šZ"•
Î?ïÓ^rÜ?pøŠgºàÏ?dŽƒ$??d"ÏZ`;²?ho©=?efà}du?ïȆwš'?|£äbIÌ?fî
ã»T?aIPh霓?pEöƦ±?vº¡ˆÒR?îFÑJI?™s‹à?è›?ži¼êÔ
3?'çäób¢\?˜ÓÈè²H¢?Œ1×Oðt?ï|¯L£
 ?'Ø±€?"½ÝP¨c?|ëlc@BA?x,Ÿ)(Rç?s ĊálAGN3FGL J0516.7-6207@pø6ÀP½ˆÀAaG P À8/›fù3]À;JbýüÁ?åãÁ¦(U@pyà@)Á'°—¿ÛN{Òοãhxt…ãÚ¿à–€Ï7$¿æ]º,§ÜAGNbll?ïû±¥.?3ð*fs©k?µÆóñ¥?
líxÓ?=¬e]Öª?2/¸©<†?ï(
Ê1Ö¬?—o8¶Š_?v|Ùmº°¥?w7¦4/¦?•_V›_p?"ý4ñМ?îÚV9êÔÂ?"˜ö—² ?ƒ9HB.cÄ?t´²X]?›"˜Ë4ê?'¥AŸZïR?íµZ˜…{? ¡Í$ùn?}U®¾08?v(rŸ¶?°ÐN²K´?Ÿñ]f<¾Û?ïþ*BÑP?4¿{C?b•Èõ~@?_¨Lì0?%ÅóÂj€J?Z-.ØÓ?省é?'rgm:e?hy8ÿ©s?d5šÚùî"?€vlì
y?ÆìœÎ'Ø?ïŠNëu"g?~[£ík
?u'—ÐÁûð?kk~›ÁÝö?'Øy,''{?z¹ª—TD?ïe
&j^)?"¿'B{u?mŽž…N?Z®CT%Œ¦?zÒæ¶r?"FLÍ}AGN3FGL J0517.4+4540@d^\FR@÷QÿÒÊÀ9ËzdJ,tÀ;UÂ%©Ý´¿ä>ÏôEÑ@hú?v¸@°IÀheo¿ç²¥4M¿è¢9`ýN}¿àî«ÌÌ÷À¿è3MU%ÿÍAGNfsrq?ïøº{çW?I•ø0;F÷?[|¸?¿äx'Þo?JJ ep`?H¡'jT¼Ù?î"% mU:?µF3§2›?zã]2?†"&ZT+É?ªJwõÑ?´ÿ`ä?‡?îlνñE[?"g[@Þæ'?‰@jùÿþ?w7Xêyq`?¢âù`³Ü×?'ñ\nØà2?ïÅì¤63K?v@"À¼9?j"Ÿ®á?¼?)Tiœ?|Ä|ð—0?v0Ñ)	?ïý³ŽÚ›9?0@o2aX?
Õ$ð€V?çi+²n?.Èwâ¦?-éPI!K?ïÍ==«»?›‰v`Ú`^?aÕÔ£Ôݝ?i3s`?‹;yáiþ?™ùñ'"?ïp'Hä¯?µ
Êǁ?v΄*¿?g[%TH7Ä?ˆt+ƹT£?}·pd'
É?ïô­$wï?KI`·-$?gœ@‰R>üvXOv(g?V
zŠé08?K'<þr¥AGN3FGL J0517.5+0902@h0à?pXXÀ0)ÃÀ´–À9Æb‹æR°À:ùŽ,~
¿ä¤¤Ù$R@Ë°…ni@b»q"î?黎W4ÍÆ¿ìñ÷MB·¿Û­ðÂåC¿áä|í͉œAGNfsrq?ãÀ''.Þ?Вspÿ¶?i4®¡~@~?k¢(Žˆ|7?ØM‡21£?Аz°P?îòe²®?¨Ô½—[Ãù?}˕'ò'?'†ÜRþ¶ô?šI-ÙG¨?¦ƒëy¹"?çL$Ê©v?µ0O_˜ÿ±?¨&""ÛE?–(B'—^æ?ÌÆ"Œz×?µ.4Z"ð?å<Y˜?¿dˆD …?g°àËmåS?d– "Ç@¡?ÕWë#z¥?¿\}fT•%?æóü
y‡£?ÏÄKÀÈ?U9»ŒÚU¹?VXkØ}ü?ÒÎ)KÜU?ÏÆdØ
²O?ï­Áûsºs?‹X¯Õ¬Uš?dPU~ÉËò?dñ9++e&?~öׇmÌ|?‡hš
g=û?ì"֏ªh°?¤Ð3• ê?š$Ǒw×À?Š\)aþ@Æ?´Ðê?£XØ·¦DÚ?ëžwÕ­#Ã?¨FU'q™?aM®#1dÿ?PårK|A?Á@éîàaÄ?¨:[Ù`'4AGN3FGL J0519.2-4542@ooý¿HÌÀA]›ÿ¥g-À:QÈI°MÀ;qÕÉːÀ^+¸ën@R#½Iw@ááÀ¤ËQ¿ãMsjƃ¿è;ԓ¯cŸ¿êÛ¿Z½¶¿Ð²­3KÔ6AGNrdg?ïôÙÜw1?P
(¹lL?BæEþF‰/?BK+K¥>?LšSM‡!?EeNiÚÿw?ï'Fú˜ë|?‹-ýÌñv*?fr½Å"'?~*šÅ€»?…Ñ»žýÐ?€ÕðZÆ$?îQûŽõP?'¤ÆKè܄?'8¤û)?~
!uvqÈ?¡ÄFPÓIl?Š×'TÐß#?ﯣrFª›?'W½ Ví>ศ"oàõ>ð|Ùð'6V?"õ7ˆÿ?'Uwñs3J?ïú>_X¢?@üúJðÔ?0†¸eþl?0¡ãx‹†??7U÷b€¬?7"i(3
?ïÝà¨CLþ?ipÂ¥I'­?Pè*t"gá?PH¢§¼?i«B]M†?c–ÑÛWéœ?ïTw£Ð4?x=¯';Sv?ƒBÑs%?p¡ŠÍH%?‡ÞÔ-¶"ó?k""53ô?ïïAžÛÍÇ?X˜}­r£>£Ú€­Øßí>§wŒ`ê\ÿ?`½#"L?X—ì©›ãAGN3FGL J0519.3+2746@f:" ³Ô®Àá'_Á0·À9Ó[&—C~À;iï‡â¸¿ôËó @݅6‹,n@¤y¿^¥'¿ìS«lfð¿âö:qÆ}¿ÙÝWu9¿â~'ùZAGNbcu?ì`|Í0?ºz¦lïJ.?ƒàÝãcÿ¼?'‰x"äe?ºýÚ>'û?¹Þhëü½Ö?ìöß'öǦ?ºv›¿R€?Ž-,¹Že?"M~‡G?´ƒa(¹Ý‡?·ðª‰—H%?êÞrbI?©íÒݱAC?§C"Pìè?'Ôô¦•‹?½j¥êyŸÃ?¥Õ˜Öٟ?ìgÅù~B?«ð.†é"J?Kà"¸ú¾¶?IZ›¸äA0?¼Š€Z?«Û¿žVk?î_þôöT?³ê=¬ x?ro#å:"?rÂM€.?§¾BÕÄku?³zN†½ø2?Õ5?£)h×uki?v1%âFÂk?|ý¸I×hH?—¢3·‹ž¹? JT ¶ÜZ?îrù=²×È?'ÀæØ…?'XÄx{¢õ?'î‡3? $	êL€?Œê8§în?îÒCs"™¢?zÖðCÖ?;Ñ!µ"­Ý?0kesÈ?¢¤&…7ÓO?AŽ8~AGN3FGL J0519.5+0852@h=쿱[WÀ/°¾|§ñÀ99{*BÉ©À;šþô?ùÀZ*ÃÍö@'´#lÂ?ÿﴀ¥¬Í¿Üû¾Ê"¿æWdØi/'¿è?ÀDb¿ïÿ¾ú¤™AGNbcu?Áê>[Ê?»)"Ÿšö¢?ÕøñHœ?ÊÑiÿøô?àˆ÷ éw±?Í4d/CSV?Äí´K.?Á…YÎb?ã7Ò]k§)?ÆäN—+ð?Î3¦ÔV±?Á˜T)?Òì¨Ñ+<€?±;–äE€?Û>Øó™?³Æ;A?R‹?ÑÕH!èï(?±š° ï÷?Ç·Cù?©¯2‡?á'FÐ/>?ºÂ¾ùFõª?ÔI—–½¤Ä?¶î‰Û^?Δþ¿¹?Å}L#ø‹?Ô§õŽJÐ?ÉýY?Ü
‹+­?Ìàžä¿¯?Ñ[™×Šžˆ?ÄÁvWu1Û?áhb"YIÙ?ÄãCÏÁ&"?ǧB…›‹?¹¨Ùúº?Üø·c{qÞ?´G:¬°>û?ÖèÍËò©£?°¬ï4FQË?È<õ¡#Èÿ?«-Õ³ÄÔ?̙|¦¢II?ªR"ø؍X?âüö߁¥?²AŒ$V›?Çr§ÛY`!?¥ßŽ«7åMIXED3FGL J0521.4-1740@kuNóÀ;•sà¢l§À9ÇquŽ!–À;Áó™À0¿ø›«–ò@ÓtMéÄ@nó€jÉx¿âBå'Ñ++¿çѪÒ'¿çi ÙŸŠ¿Üç¶vãÐäAGNfsrq?îëX"7ö?©%巒Cˆ?e~2›ÂÃ{?i~rÍν?Ÿå).qÀ?¨¥"KA‰ó?ïnXµù¡—?Cã¹á(H?n©8ÚE+?mMT'Éé?Œ¿"ŽdÜ?Œ4Ð$?í·µ[ln?›E©â¤ëÖ?—#Šå÷W?ƒÉ»öƒ˜?¨òäÔúo}?•m$åuaÂ?ï=Q[V+Ê?…"ÉkŠ?7ckøè?=ïA8-ǂ?—øFò.t?Ž÷…ps?ï#PÁR_?¾ëÍXà©?M˜;h:?TvŸš•½?š¬ó
ŠIs?¾ÒiH1á¾?ïÏ´Û`Û¯?sÍPºƒª?Wò9®x?X0' ë?r)ÐÀc?oÔs'Ê{º?ï7UJpwÈ?'Â%ÕØ´??ƒGz_¼?m,ÐùSÂ?Žã2ÿV˜Û?€XÙ¹??ïÞeu…?e–	¸¹?	$ù¼~,?ÛØõ?pšüc‰?dç&ؘpAAGN3FGL J0521.7+0103@i)rÿÑÜ×À3T‡`±ñÀ:5:¯(wÀ;š#;nk?ÏœÓ+¼@pÁFóµ?û-€H9Ö?îâw]•Ä¿Ó"¨)Ãf—	'›â¿ÇEnbøâAGNbcu?ïú%=@?E‹XÎ¥S?&¯¬ÀS5V?"Ѿ•Ûˆ?BG€Ow2Ñ?BAºï§¨Ö?ï`‰åòb³?"«Ð[€6û?q^sgӑI?u–BSI?.LÓõv?'žjHO"s?ï
ÚÅ͘é?…^!U7?†Žsó-8ç?wCí\8¶è?'ýmJþxc?^ ™pŒ?ï­uª¸6?•øñëU©?PÛèÔÙKa?YùmSed?žÜ'½‡_…?•¯ëÕ _?ïüHi6‹"?6B3Ôû¬7?íRw	Oç?û2ÿ²Ò?6Ac´Ù@S?3#+ô0Ô?ïÌýÍSc?u	¢ç†A?ZLº÷?ðŽ?WIB[r¬?ríê¯+ì3?q¦Þ­s5ð?+Õq?s5©¯b?ý?z>öcL•?iiZaHbü?€ýì¹Øý}?kH;Á1}?ïÉs»RjË?pW "9XÄ?GO³µ?A¯´®&ä?x\+褹D?oÖhX¹<"AGN3FGL J0521.7+2113@fó'àÀ!gž´JÀ7LªÓ}ÁÀ:l²oStò?Æp^'ê@ëH>³?þĤ_E_Ü¿ÜÙ©Þ¿à
õò"Žp¿Û°Š¡Ú¿ÜSóÉAGNbll?ïYô–q?š*CÆ4t?B©‡¹úc?P¿^¦Þ¹z?"0–׺"û?™ßåî?î̷ۘuš?¥ ±á›S?y¡Ÿ'p-?'"?ðrç?žK¾R£«?¢Ž6<'¦'?éÐHàÍv?³¾ÂÂä"à?"góªU?‹SĭÞ?Æ^¯|ž¥â?²ˆÊô˜^T?înaªófÈ?™Ôªـ%?6›V}ž]9?=«]?®?¨ì®£ó¸ë?™Æ'Tnb?ïá»ëÂË?xÝdûM?-lME뜭?/œß"ZgÆ?lmO&—c?x~zÌ%eF?ï‹î'\ݞ?'øòHÆâ?fŠÀû?gBA~/œÚ?‡€ @³Â?¯Lv'?ìÅÅãk0?©¹ßÇ~Ä?‹ëRè½ëŸ?‡|"îŽSð?¶Tm'ƒŽ?§äÿ¯´IY?ïm‰J8Æ?|²h#&4?-5áF€Ó?$À™ü½%X?'jòÇp2?|±(†ýÏÀAGN3FGL J0521.9-3847@ni>_·¼À@­? (ÿÔÀ:?³~G-¼À;Ç?QN§-À¬âF[®ý@^VYS†@… êÚ¿í=ÌÍ´ºn¿áƨR⌿äì~9R`¿à".¾¯SAGNbcu?ïþãšï…	?&k4Öä?à°Å('?k/t(¸?œJ¶ß˜›?•+
uŸ?ï™4xò\?‡¡úâ@Æ?e°£avô?rã!Djµx?"F¹8J"/?€è¡¿'âH?ï"%šÕj?"¾âr^=ä?ƒCã/hç?t£àFàÑ?'[‰õi?~*̆OÁ?ïõ"Ò4•´?WG˔4U>¸{kp«ÌO>È©0
…i?TÐ<Ö»‡,?WF;ÕÄo=?ïÿ:‡²³¾?Tʘd>÷7RV/ÿó>ò&¦c'f?á9Ë°R¢?˯;‰Õ?ïÞ5–ÿz8?i×wÅOÌ?PeÄ ›z÷?Nh2¤j±?i—†žZ¯?d}áÝI)'?ïh	˜sî?t§¤Ì4ê?saÀü=_}?czÇÄì­å?}ê:If¡+?qÓ¸ü¯j?ïþsSðÔ$?'TxŒo%k>…Š0Åë€>§g¯úƒÛ?(Åa¡†—Š?'Rû´ŠãAGN3FGL J0522.9-3628@nð`»+»À@[ò¿¥œÝÀ7ë×TLÀ;$†îœ*n?ðZYŠµÑ@æÑZÑ@/hDq¿â§ÝÖº}¿ç8Á5¦\¿ç%]Àƒ¿ä}óKoG¿AGNBCU?ïù¢ÓÔþÊ?BBA?7ñSFž¢?7¬!îÞi?:øû=Þë?4>üG÷Ô?@·Í"?‡'äÁµ?fÊCá|?f²9ªnô—?…Ó½a1ä£?ƒ8Ëv?^8ß3?"ù'£]?'â
\ái?ˆ*q'¿dí?™oR,Ïj,?"}à\tì?ïÃOºÊ¹?'¢‡`¨R—?0>s'JÂ?C«ý‰UC?}T;_ŠP½?'}ø!ñŒ?ïýîÓ ¾?*0óuÑ?%çhô||? "y+b?(‰­wB?e<VÒ)?ïÜ\̬
?ku¤w›?Qÿ:ãùµž?PÉ~]+ëÈ?j£–æã?eš‡ßÁž×?ïE²l·?ŠÊ¡ø™Ì?"ývLè…?~è$\¤ÈV?‰–uƒ×éË?'±)oóR}?ïö£úó¬?WÃ÷ݺåS?‹¨†ÛÆW?Ý]Íèì?QOQ‹à¶Ë?Wa¹veïAGN3FGL J0525.3-4558@o}Øÿu–…À@Ùr 0ŒÀ:VHø"À;Ù®&ïX?âÁ©\t	@Ñc	/ª@œôBp¿åØ ¬¿â	õH…Ä"¿×suéOY¿í€±b°qAGNfsrq?îz ¯€"?£oÏQ'?–!ž\ã5
?"Óí=àª2?šŽ=‹têm?Ÿ´š3Äê?í?/5«;5?®S•c¨?›Ä*%"C†?˜MÓdÒ¤?®*÷"^'è?¦\o(Ãê?êÓ€Uç?«GòÅËIí?¹Òè+R›?£CUÜ~¼6?±¦{ÑZñ«?žv]ðÅ&E?ì¢è÷½Å?¥"P œ?¡t?
4"æ?–¹!Ê*0*?². oùi? ¶"-çà?ïûë¦à?˜<8çébú?Š®øˆM¨?…Çöꦩ,?(|×a+?"èUœóø?îýÁzðÇ?•ë—€IBg?‰Ë»ƒ7þ*?"®'FÝ-D?"aòÿµ"?'6èŽ8?ì÷µoÒº'?¢9»GD?¯Lrf¨?›–¯:‡é­?¡)¸¾@?'ˆ²2ñ?î¹SäŒ9½?ˆÛ©Ûò^Ì?˜4eëÊÇm?€—/Ã"eA?¡‡Õjä?|k+pçjAGN3FGL J0525.6-6013@pÑ̀CRÀ@ïÇÿÞrÀ9•üÁ‡mÀ;zšéû±½?ñμI¢á@EpOô4?ûžŒÀmBù¿Òæëˆ
X¿Ü2Ýð-¿"œb2
zi¿áD‰8ð®ÌAGNbcu?ï"/#ÿY?‹R{œÆ"?wR Üçö—?t6Š'¤d?ƒJæÑÛRj?"\ ­E±-?ï´hÛiP?šä­Kû?~iq΀w?'¯Ðà{æ?˜OxhÍ?•5:?."¯?ì¤ÝxR?©ÅCZ‹™?®Ì"®°Ëó??T\VJÃ?°\Ǿ0ò?¡aYbý
M?ìõæò›q?§…såÞtH?ˆðÜ:lÒ*?…I&JÔ?µ2¬åŽ«"?¤®´ÛTÕ?﹞0Ïx?|€‰#‡ö?móF1àFU?fWŽ?t7D"#C²?un%¸yk??<©‡+?'™t˜FÊø?nÙÿw.^²?i<7wë:ø?€ápöÊ»'?}"1ßlÕË?îT\֚«è?–Çc F.?›ñvüëáV?Œcyp0?™'î''›¬?ŽvŸƒ8e?îÑ&æ@3?'ºî†Žƒ?þ"Õr?'m4¤âùæ?•ÞÍQî9x?†LD90qdAGN3FGL J0525.8-2014@kÙq`•l
À;ñ Á¬À:[ìSzÑWÀ;ß:ZMS?–PnU_È@zû¸G¯—@€V@(¿×®éö0üÖ¿á¹u«dš¿×ˆ€º¿èü·•FèaAGNbcu?ïîTOD"?\5"'Í…?OK×éðq?T,j¤1Ï?S±vž"Y?N"᢫·?îêtª™=¡?Ÿà¸?‹¬?' "¦ãš?€E" >R?™¡(aщÔ?›Ó
î4jZ?îÆ=«K±?uàkŠô'?"jD.'–n?ˆ§Ó²ÞÓÏ?"ÎdœW|?€ysŽãø(?î[##'ù?•NU—nîŒ?{«óó*?sÎçᨊy?¦ëøDÌm?"«Jƒø@Æ?ïápÚwt?ªLb"üÌ?[O\õ$Šô?™\dÕB?`çvÉAqI?›^£Ýþ?﯀4"?7élêàÆ?fÒ&ÓÔRþ?_0ŒŽ½ùB?},{ÍŊ?{,N©7œ¦?ïiÂÒßÀ?¦ŒÎw—?""Åí¢"Ç?@¿;Ù¼?
…KÐ)K?k)2/¨fG?ï•&Ø(lþ?t"êÄE¤?jÔì0‹RJ?Tº˜ ?"â2Çù?r7RGb¤—AGN3FGL J0526.0+4253@dÔ_õI@Ã×Àâ¯À9\sв4›À;SÕ™êø?òmJ(B>i@óa4Î=æ@{ðà}XÆ¿Ùm¹,˜­¿êzôE•¿åÌ
ÏmÞL¿ïÿàL¨ÇAGNbcu?੟|,2?ȵº?4&?Ìp/AOðG?Ã\ß1±Üd?ÐtªR_¯y?Ém¿åÍh˜?Êk›ô+¥?ÄÚIçCŠ]?×IQ\©_?ÃMÞ B{â?Û¬ù©@Î?ÉoôšI²?áL˜ÊfÀÿ?´G'»@ù¾?ÒnÑÖDS?±[¸ÁO?Åïù*Vs]?¨,Q–Æa–?Ö¯Çû¤?°ÎÒÕË/0?Úrx"€ø?¶°/>NH?Îù°MõÕ?­%Ÿ
—"¤?æR`–Sû?Åð"ÒO?†÷Ç]ˆX?¼V¹±MP§?Ä/…áxLå?–…í.0?ڒ=ƒy¥?Ȩ¥™4Íp?Ñ앑ąx?ºÅ×?Ӂ-a¸ã?Å%`¦w½?ç±99÷6r?®Œ€dç?Æ10³•Ýç?¨á±C+?¶ÔÈ>©¦?žŸQÆD"?â\óÉÄbN?§R›ZT?ÓýˆüéJ1?¨ýÓîC?½"=¾7ÄÏ?›'E :vMIXED3FGL J0526.2-4829@oßU>öµÔÀ@àn¿Ñ;ÇÀ8Êû¡ÌnÀ;\¾óÆ5Ú?Ó¼0ýMô@N˜|äG@NR@i§Ž¿âÓ»Ôàu)¿ãÏ¡t?©¿ã"¢3ž¿ç…l1g½:AGNfsrq?ïôô˜1©_?MÅO—(?1øa8??.Øï!Yð?Q˜ËWˆd?J¾Ʋ™?ï†ëˆ"{·?†ßçáÅ;?f˜½yé=?f'7`½?ˆÄwª
Éë?".¤ª¿;?îëO»qH?†ÐƒJü?‰k¥0Øh?w
bbL…¨?•à6jÂ?€¯ƒ º?ïqíí¦.?†Éß#êÕq?HRiŒö-?Grý´Ã÷?'îð…†	?†B%s?ïü3ý³tŒ?4Ià5t‡Â?#¸ë.&:_?$cXŽ½?¸?4ƒ¼ú
‰?,ÙQã§Ør?ï×V™r_÷?m´¦ÌÆ4]?TÛvHI?QÐÈdE?s?n;àx÷¼?g.ûpš6?ï•ç¦íÀ?p_·a´ÝŽ?vIuÞ_6"?f¼¨±÷HË?&–?»z?dZJoT ?ïáòYµd7?c(!+Ó©D?4·ô7ÿÿ?*"dÓÝ?kv§Û]©?b«:ŒŠ AGN3FGL J0526.6-6825e@qm~KZÀ@lӀE4½À6_MkÝyÀ:?æW¸Mº?þOI"H¢@èVÁèb@u°Ÿoœ¿ß¾Nî÷ð¿ã7we'+¿å³ß@¿äÂôÁÞ\AOTHERGAL?Î<ÍÑ.±C?Ä_ö•sR?¿Ô¨ù³à˜?À{›!."þ?äv7l}ל?Èsê]ep?ĵ…k'c?Æêq‡pû?ã{n	aÂ?Ì»Ñ>˜ä_?Í^
Bnö"?˜mn1OÈ?Ô^þ"v?±Ù[À¡ït?Îc¦ÁRù«?±9u€ä?Üo.
PíÑ?³=@";?§ úß2??›Rþ0›I	?Û$Úyw?Ãô~—Š¡?àûÓˆŽë?ÂÞèùS=•?ÓûÍèø?É9ÎÃG
?ÅÓ&ì[þ?ÃÙ-3Ðù?àn^h§E?Ëò*ŸÔy?Ç%pc%¥g?ÇQçÌqL?äÚ̃¯?Ê#vùAÛÿ?Åo]©ÛÜ?»D×NÊ­'?טÛo6?³Jv$z?Ð,íb³B?±lZó]ޗ?ØW¼7†Ýˆ?³ tˆ Ê|?²Ì"·,|‹?ž¸´ÀP7‡?Û½ßwŸI?¹0)i`	ä?ߏÒ3F±ô?º'pÕw£MIXED3FGL J0526.6+6321@b"™Ÿä6v@.†þ "ofÀ9úÈ×'šÀ;͔ãQs?è
™"GÊç@hfʺMï@Q·fw®¿æâ?j¤
¼¿ãTR+Š·¿ìJªó€&¿ïÿҁWèAGNbcu?î»±¹mká?§¯GÎó.?¡<tQ?ö?¥5ÎÜÜ	b?xC€Ý†ëƒ?g/Týkz?ã1·véU?ÇñÌlε?Ѹ^ß<?ÁˆgR8?Á/±fv|?½40&l?ì/úNî®'?¥·9|G?²Ó{?Jõp?ŸÀe€ûL™?§Yd•ç²?•!¨üuøN?ÞfÕHé :?¸Z
ã?Üm.è±ì?»
ˆÐZ?µêöõí?¤÷"Ußf?ït¤ak!Y?¦¡^cQwÜ?‹œgCý`?¢7X–KÕ?lêk…ú?†uKÆ*†?ë°êV~"?·ýlm_«—?´.Ï%Œ?©Ói­"¸?«·R8ÈM«?­g…‰Ð?îHž…DU£?'IÃØ?¡õ¸òWÿN?Œ¾_F˜‡ú?"½t}?%¦a¹ès?êb¶¼È¦?¤´Ä¨	ê?ÂnHI½/Ã?¡Ç
[cc? &ÓhL•?'ò¬GÍóAGN3FGL J0528.3+1815@g^·`¿]yÀ"d²—À:s'7ËHhÀ;™;ÞÓ_Ž?æ5P÷¿>Å@qZRÜÆÀ?úU{?Œ?¢eÉæñ勵¿7¿8Sr]¿ÚäP¨u:Ñ¿Æ¡eÑýŠAGNbcu?ïÉ\H
?u>IP†v?WæÖȪýe?SÍ%Ñå:?uX&EÀ?r'¸ßÇÂ?ì‹çs…øl?Á/=O8D?'±E¹›ã8?–û
DHü–?¶ôrôiU?¾iºe?î=LG	—?•Áüq('?'²­Û¨¯M?Öž€ˆÏf?¢Ñ䡛>â?Ê¬(jìÙ?í:z´Ém>?£S¦Êsoþ?–5›V?'ÑœÅg
£?²yc¸%? Ïµ/XO{?ïãóþÑ?cU®ÝÌm?FÂÝ{¸?Aƒ7æ›Ä?f[IÊã(?`×FÌúá?îÐæõ—ò%?©)š[ 	¬?|ÌéIÿA?ƒ[2iSh?ž¯çå?¥ÖÚú"br?ïNR?VÆÐ?}"
s›ã?™é–¡2?m4P­U-?ŠÑ†™,yj?w+ˆÛ)?ïî:ތ?‡yôžß?ƒ?ÆÀâò?|h—"7g?'bU¼sY?€ÒŒèÐËIAGN3FGL J0529.1+0933@hSvÿ:Þ"À*è¬A<
rÀ9fµ¨ÃÙÀ;DBì䚿æ
·­Å@^&ˆó@ˆÏ`zê¿á[Æi¿çœÏ2å[¿ìY "Qº?×0sêwFwAGNbcu?ïªl§6ÿà?'‡$Ÿ¥m?ywN]^"†?'ìÝà,½Y?qR^ÿsE?…5zÃè
?j¶‡?Œ?x‹¸øˆ?nM¿]›å?rã€Í­¸Ù?ˆê3(?‡%¼^1çî?íÄq¶ž®?–жy`Ô?œ^žÙºêú?‰‹Ñ>}g?¥‰•&®š§?¨3‡¹>È?ïLZëOC?"=…e'Óm?#œË5qž¢?7èX±ü˜ä?–Miõ^ò?":i_†n?ïæT&Œ |?g† ^¥íÝ?Z$®µ‡!?[¿Y Èös?Y3™fÄ1T?XðÕ~@à?ïÓ
‡¶B?xu=""-?X@n
dÕ?_wéŽ)?pjÓ~.é~?r¸ŒÌõ?ïmN7ž?ˆ]*Mg"!?Šî^Aÿª?|°
y,z?ŽŒ¾
 Æ?€Q…Db?ïâ3-î•?k¿ŽÐÜ´ž>ö*ûùµ?Îì^pÂ?mÇvֆî÷?k¼^œÚrAGN3FGL J0529.2-5917@p¿j€JÀ@½i@5z5À:\(^ÃÚ¶À;Ú`S&ÛSR¦¿@
—>•¼ë-@ÿÜ TsË¿èüî8ég¿åuk—RÂp¿á\6°§cm¿ØSrÇ^AGNbll?ï™Ñ~Òâ?&'9è?JH~àž‹
?HÙÈ*Hv?‡çOšo?Œ;ûk®?ïk—"&Ñâ?­ö÷,l§?mæþûh٘?|ùö¡x? _'û)?Švù	*q?í¼å0àŒ?ší×BùM)?•=½ü‰Û?€Ð¥h'?©¡-Ì;äO?•¶RÕ€0?îö;œŸn¬?‹‡PȘ«J?SÜfœcòÇ?Uù¨¡—
?ŸúÆ	ƒL?‹s'P76?ïé±çe¡½?j´Æ³
¢?3+jöUZU?0{œõÛ·?cè«;Û?iNçÇ'ž?ïÐí/T?qävüôÐ?Wðá)%=Q?TR¬±¤+?qýÑ3Z;³?mÅÓæñ?ïDé·¥Y?z©ß8g?€ÒZšÉ!?d¿xùV?Ž'ëq?t;yW¡¨å?ïÎóÕ>$B?dz›e@]~?=™{f?7?2–OZÀV^?v¬}ª+^g?cq®1ð׳AGN3FGL J0529.8-7242@q¼¿šÏúÀ?×ÇÀ'áÀ9«èYM‰À;ªÔ}›6¿úhßè]vÿ@/€3;@ÌπsÝ¿æ^ï_Úí¿ë€ [ՓƿԬ0ÈÓK ¿èü2•ÿ[AGNbcu?ïþ8,lD¢?&žÿû›®>óäx×ÜýA>ñþ—âm†?*¬Wjw÷?%µ€€E)?T³Ç©?…püõèº?gØÞ-;ZF?iszÏÀ¤K?†ßs;¸(?ÑD¸?ï½ú:Ýæ?…™1õ'?z²M!øI'?b×äâ£h?—[­ižîÝ?"¼S?ދh?ïË!Iëu?r¹Á©Äd<>ýÒHŽé¥^?E!?8š'?zZœðò_?r›	À¤ôŒ?ïþÈGR?³Òê´\ã>ø"Ö''j>õm±êe²? yÓ¶5¯?¢ç÷òY?ïÚú²ÁÓ?iÞ{"[s?RIréÅ>®?P׀_)éÛ?kà"W ÝÔ?cýy½Ü?ï ßO #?k½~¹	±?lQ!®ò€?O†àÈÄâÃ?€³ã 7"K?hùçb|X_?ïöÁIÅy?I_–DÐÁ…>ãûÊ÷¡>öDÔÔ¼Úx?RW`Á?IN¼^ŠYAGN3FGL J0530.8+1330@gëü–þµÀ&‹$£MÀ7ºÇªÀ;ÒÎn|?ýËk[BÆÏ@._@B-¡ú¿âúžrœU¿ç—Áf«õV¿èêPⲊ¿í'H¶ÁâRAGNFSRQ?ëÃÀ[ác?½£t}š#q?·¥ð­BR?·Óðã,Š£?¤'r¢¿"?©|K©¦6?îÖ¸‡à""?¤CpÉ¼(?ƒ7Œ'øS?ƒ}²€=è?›kD
úS?¡'…Ïr?ëÝÜlÛ~?ª–{\Ì?µûÓ¿a(?¤÷±>0OD?¦+ùˆ5¦Ò?›²ó'—ƒ?üðJ?¢¥â+t?M%ø?'f½ÁqC? dV½b1à?Ÿ{WPÜ?êÒ-j$¹?ÅVL"]?¾°Š)—²?Â`¯ô‹ÿ?¦¹ÈIk•?«ûüØ[µÙ?ïˆzzšzë?‹}m׌¡?q¸
‹£s¢?mÉvœ5 Œ?…ZŽÀu?†'kß	*ð?ëÁ"~–wÀ?­wô«©Šª?¶Ôƒ2¹‹ˆ?§cÛJ'¼?¦=±³¹!í?œ¾ñº9o?ï÷ ¤¿?ÊZØAã¹?{e®ÓäE?rÛNp''´?|‡îc-?{±v7pUèAGN3FGL J0532.0-4827@oà 6mÀ@g`#VFÀ7F™¦.ÓRÀ:¤"Øi¹?ö¨Y-æ&@0¿»lR?ÿ}•øÛI¿Û¾òˆ¤¿â—:·6¬¿á;—ÇB°e¿å£^™4ç5AGNBCU?ïî±zš·?]7]'C¿?7¯·ý­¡V?5õ#	Z?\±¶(Ú	?[¬'9×?ï˜"B­?ˆ‡@ìþGN?cêؑ`??rÜV€àÓ$?"üÜæɘÓ?'h—Y€?îV6MÍpê?™dN»Dñ?ˆ»zê×Ð?‡*´n
"?¢X=e³…u?"!‹—­™?ïð¬|[?j…<¤"ïü>ð5;[GÀC?òqD§ò?_¡ÑÈFl¬?ju锘MË?ïúbb(qÂ?BÛÙ<ï5?,êbžµ\?*÷B…ø.?>á{Žn®?>Pœ§¨^?ïàõú©»?h¸:`"{g?OWÙÖ¤ÍÝ?N÷dzà?g4ߺC?b¡_´7)?ï#M ˆûV?ŽÇç‹?††?{"@¬?83s°?S<9­zì?†^l–À?ïüòÍpl?B9Èbû(>äîî¬}ޟ>ðœKhÍHÂ?7ÂC®?B´tAGN3FGL J0532.7+0732@h›5'Ì÷À+sóþiýËÀ7|äJ7\À:ޖstkã?øVV"÷@ʖpÅ:@¶¤¨ÁTÊ¿á^jL¶"M¿å°?é$h¿ä3Rè°-/¿è6¦¼þàAGNFSRQ?ïïWG\?V&j·&Çé?:€
†ü½?;˜ŸÂß7?[7N¬#Ÿ˜?Sˆp*û [?ïu½
P՟?Œパ}=?r%Á&n³K?t…þ.1'S?‰}ÜÓސ?†>Îá"È
?î£Ôm«?—Û'B?‹¬w5ÏA]?Úïr¼§?¯4nC?ö?'¹a´E¯q?䀘ȅ{'?"è`XÁ?@;,j¸{?Q'c†Ãl<?"[
²8)?"ƶڳox?ïøkà_?DÙÂYë?2ͳèDÊ?4LtJF«?D饎äÎm?=Á¬{æÀ?ïË@£3K\?vÄ9ºÝ?[‰F§·c?Z,'Wˆ);?s}\ÏrDD?qɳ­ãóÆ?ïO-:ÜÛõ?†¤/5&ò@?'4Ã¸FÆ?v"¥{ƒ?Š/éR?AæúÍ?ï쪯…X?dXÚòS?5ŒÞEIq@?9	ǽ|dÓ?`£´Å'ø6?cpZ}qgCAGN3FGL J0533.0-3939@n˜¬B»fÀ?d;ߪ#À9îRŠçO/À;¾ê·™^áÀš®ý®í@A
;|Ù@æ½ÿ|¿×¦¾laÓ¿èØKIeµÎ¿æ*EEPäk¿á_"½'"AGNbcu?ï콇×ǟ?^(¨Å {	?Kz÷õ¸If?RtG¿û
?XÇtª>/û?Vl÷Ö5O?ï›ö½ÙaR?'¨Ûw¨·¨?dôh`±Þ?fr>ì…ø?ƒÅ6pùi?Äô-5?î@–¥XB?'CÀ¼K´Ú?˜©öÀ?‰I°c»?Ÿí$¯W‰
?‡%ËÛO
n?ï©Ä~8ƒï?ùGnD|j?
34Õ4ó?t*¦•K?…q­DÛÌü?åW6¸mÙ?ïÝìÌ5g?¬rM§ãX?i2Ù$;¤?¨:ߎ–<_?QÂGâé€ú?€å‡¹\T'?ïڕ4°
õ?jz &Eúä?S7Š–SŒm?Q¶ØÆ'?kÏÊ"?d¿h"ÿ?ï?&¥‹™?†ÅwDºW?ˆËƒ"im?'¶Å0™£?‡jӑÃd?w2|6Ñ?ïðä{V?V"<Æ+>Ò¹+˜y9Õ>àÕtÙYÍ?^$QÉÒF?V€QýìŒAGN3FGL J0533.2+4822@dE$û¨'@ rE AYÀ8uŸÕôÀ;<ERðgÝ?ë¨UTxÛ½@f»ŠPG@__áçç¿âå¬H·˜¢¿å±'ì>hW¿å•™(ýǎ¿çn[b¹fAGNfsrq?ïîÄÁƒ›?WÛèÏõ?MÁô w‡?H¥€Þ±Ú?S¶›•Ä¹2?P,î¡fu?î·Z'÷?§aí¥Û'?{ìº;BPÓ?{Njôyä?¡SÂ7o?¥þûé²ñ
?î}¨H¢Êß?"†ÍV†?'k.¸VÛ?ƒ$"ýQæ,?žßÈ3'M6?tj‹;'?ïFW¢Ô*å?ç
¨¥Ÿ8?h/D¡ƒ?h|<…Òt?"#íL&?ìÛq;"?ïú#ÄD+î?SâÔ‹Ö¹?:*4fWÛ?M斯$â`?4·¨ p+?8}"×!º½?ïšæd'?¢?†¶L¶D¨¯?faŒÓ³©å?bJ™Q&G?ƒ®­º[?"=Ì"B?ïQoƒgöV?…WCê­¶Ç?'q¡@ùª?y.¿{l?‰2}â¡"å?}ºÁô·æv?ï×TÙºá?p‰Iã¶
?RZʞð«¯?GØsõ˜?o¸F	§7?p±1FçAGN3FGL J0533.6-8323@r|˜`fÀ=&7PþÀ9Xå™LlÀÀ;š¬±¤RZ¿Ë,Ž@'á@æ±÷ßJ(@^*€J¿Øcî‡1¸	¿å\"åX<‹¿çåD¤Ž"¿Ó†fŸNí×AGNfsrq?ïú—d¤ß?9I~a);?,'\S9Ù?(5CØ>¿\?<û­Ú{æM?3ŸZ÷ú‰ð?ï—üÙk?"þ+ÊÈù?eAâ_p|å?eəb!hG?"ìˆ^EÌ?'þê»þÿ?îëã¼¹•t?‰§'ÂSÜ}?Žæ¸8²?'‹+bŽ,?"ƒ_ý;?}iþ6'_?ḯ(Å­/?wx2Záô	?@a6;˜"?È°ËbK‹?xâj
ÿãÌ?w_'ƒ¿Èñ?ïýrç©?)÷^ҍ?í!ê(,æ?̀"ͺ?)Ú󐮧?"ëËÕAY?ïܒ`þÇ?iÕL3‹?Q ®ÕÂ?PI§jV‹f?j¥ÅP×?dQ(2wv?ï'hSa¸?y˜úoc&?€LÞ7%Ú?uH"†˜?~<¥çG?ih‡oL?ï÷æ.PS?M†[€OÚû>þîˆhÈÓ>ý¯˜	V×"?OoÒ¼¡µ?M,´åª¼AGN3FGL J0534.0+6759@bÄupÅ@22g  ‰xÀ9_UÅ.rÚÀ;¾ÜÛ7ɛ?ù¿y'3J°@`ñz¬¢?þµðØÜö¿ãY©Ìíƒü¿ÖºØª6Ûð¿àEåÝÙ©¿ë}™–ȦPSRPSR?Ã#5lÑíü?¿L×oÏ,	?êú‰ÚŒx?À'Æ<(¿?~Teq™¬V?~¹!ˆã??Õ¤ÿºqË?Ë#ŸÐÇ?à'u¾üˆ/?˨@¦cW?Âp)'Q,?¾xùsžÞ?ÒÄÂ<P?´0¸­Ñ¢?å-aæû?´ûU>*G?­§›n«»?˜Rö±}?áæûRœ?¹ä•'	=¨?ÙCGcZ²?º&~
"?²\nÙ¼W?¥"\Zø3?ØyïZ-?ÍÖA'Vg?ãºddbß?Íêáuø?|¯wˆ¹"?wOÛ·*¶þ?Þ¤oš†m\?Ë$³WtŸÔ?Ú¡áŠ&½?ÈEu¢eè_?ºæ»hÿÑe?µÒS'ïÉa?á62Â?¸ÿç"mÑ?ÚâšÜ\.L?¸)tÜ·+?¥‰ÕóP³?•±´­/4?æqÈUõj?¯h»®«õH?ÑÀìdÕÚ?¬[˜-é?•¸/'?¡–›ÀîÑMIXED3FGL J0534.5+2201s@g´ßݵÀö@8ªAÀ7®X¡UPÀ9×U,'?
?êy@wƒ3@dN>a@Ý_Ù.…¿ïÿô!O…ú?ïÒj WS¿Ùeށ*7¿ïø¢©Ô$OTHERPWN?ÔLV¦'
?Ñ6	–£?㶐§Fo??ш§ý=5ž?± .È?¶î¸&|?èç'ï"¯z?Òþ¤QE?¹hƦJµŽ?Èæ{õn×?¿Z©âŐ ?Æék¾êáá?݃˜¢	?±å/ÂîÛ?Ðb‰¨ñâl?¯¬·–?Òݵ
?°µ­¨BŸz?é"™Õv?Ғi3Ë3›?Ŗ—ˆ¿¤?ÑyKEy?§…ˆAaÝ?ÀÏ9cŠ$?Î1X¡›Šy?ÎPÛHÕJ¹?ætÖ&p_Â?Ð ‰ªZ©f?¯í;Ôü?¹œlæ:å?ê`Jú5vë?Òí]2'?º%Dü§?Ê"ÀĀÎ?²Øc3ûú?½~÷Ž¹¹?ݾƒ¤Ëâþ?²¾~靛?ÏÝ È?®tW[T¼$?ÒRùÏ0̞?°Ï#R
Pö?îr¬uÇàÝ?¶'y_su? 
Qô†©?®¼:D ?'n\œ;Ÿ
?¯ù²vôÎÖMIXED3FGL J0534.5+2201@g¨`ܹªÀ_?«'"À4V8/v~À9D›	Ü!Ô@‹u>›q@»7»ƒ#a@§FÀÙ¤w¿àï÷…nP¿ä'ÛÇ¿å5Ò$O•"¿êÆB9`sÞPSRPSR?Ùe¢½jëB?ÏÙݒ¨õ¾?Óvèø…?ÑjßO0j?Ó#tJÿ¹?Ï-ó¶Ï*?æљfT.?Ґñg?±±¤¼¥?¸pÈ'7?Ëáٓã*?Îy¶ÃS¯Þ?Ôº Ô2¢?¸"#부?Ñ1ûAÌ y?¶Û‰…Ó¨¯?Úãë*
£?¾­ˆ±6f?ÐdÿZàî?ċ$|È8Ð?¹7¼&XÑ ?½U+•‡?䦈ÍÄn"?ÉbÍXý‹ö?Ò¦*æLi?Ï8"Jœ?ÑC&3# Ÿ?Ï_ò.?Ü®æuâ?Ò轩CZÉ?ãA·œ}¾a?ÔÆ_ý¸õL?ɺVR?ËAB"MÇ?Éàg7¶ix?È/à ò²?ÙâKç?·† öàJ?γ©w!?³ÎÓS¢à?×Û•]l?ºœô5$,¹?Òöìú®?Ãbß½í?Â%Ç9åÔÜ?»DqZFƒ®?áûŠ%
r?ÈXþ #XlMIXED3FGL J0535.6-2749@lö²ßP]À;ëÃà•®À:oGÆ;À;ÇjM{³Ö¿æ®S+z)@
"½Y'B@Qç_u0"¿ê=:þèÜ¿æóh±´¿äÏ\wWØã¿ÖàüFYxAGNbcu?ï´W‰Ì?€…þ‡†ÿ?SÁ(×?RZáô	{L?€…È83ê;?€H¡Æmþ?ïlN@ïx7?'h
çf"ƒ?qï	ž?øií´@?‹ôçAC÷d?Š¯.œq?í€îû{?œÎñÅH¬¿?˜&æ)ÝL‹?'¥Ÿa¸ä?«êΙÔ?—ßîÙ
I?ï(̙e,?‰B9µŽ?G<L&4mv?JeG'Š"ö?š,Šw'³¡?ˆùe	®¥P?ïêyœŠK?cÚÐNï?>™uyCœ&?>ÆJ‡; >?a³4ª<Ž+?a¥ªV#?ïÏ3%W?sµ×8ȵÇ?Zµ§Ëú²?`0BžÚ°?qÌ|¿Ÿ	ì?muö³òQ"?ï+d˜ÛÚ?aV5±‡¶?"jÀ+ifQ?pP~!Šë‰?ió^'úœ?u"ƹsçÌ?ïÙ\ÇEH?bYÅ<	n‡?+"È>f?!y!‹õ›?rtÿ‡e^±?b;ÉßÑoAGN3FGL J0537.4-5717@p˜Ô_õIÀ@6ä?°8À:q6Ô¨À;Ûµ_Ƚt?×35/s2@#)@oòä¼®¿ï¬qó''?å+ ¿þˆ1¿Ùé+(]þI¿ß#Ú½GÁAGNbll?ïújò3°ÿ?<Ù\œ	c*?,ÿn;኿?+	ÒN%¦ö?>(µß/å¦?3ïb%¸ßf?î÷™"uðó?Ì'1,?}³7eÍ_?'¹lôüÀ?™  e¦þ?™·ÈXÉű?ï*´é£"'?'3¯"^š‹?'ÝZn¸?p!́?':Ó?́u?}¡¾'Ëø?îû¬þȔÑ?"'ƒ÷Ë?‹T¡€‡"?ƒîÙ¿%ÿ?'àSR½†?UzP–)ÿ?ïý"G¨‹$?(~Õý@xI?²r!ü×Ï?wqz(®?0A'º"Á/?"<l'?ï¸û°KH?|p¶4{¥ò?c!]8cu{?]<Z³?yñyP6?wë¤Ûä?ï™ýB³s?rã"Ü·"7?uÙöôóÅ?hȶ#PYº?}(jã'Êï?iÃc靶´?ïÀ¤ñø'ˆ?p…{û¼?p0¶.ºM?[bܵJi¤?o.¬C'?hèú°†­AGN3FGL J0538.4-3909@nŽ@îÙÀ>E`IôÀ:SÞKzQÖÀ;Þ|WisaÀf©!¡æD@¹'ùïÔ@S–‡å<¿é	ܘġ¿Õc)%úKÇ¿àðº¤ùk‰¿Ý1*Ê®å[AGNbcu?ïú â›®?:í\IÓ\D?!ùNëô?>qu·ú?Bþ!ø&PÈ?8bÉ•Z?ï"úîÉ ñ?‰Àðsæš?h9ïªeKa?thÂÊ]j?"òÈqäÂä?'QÚë)ù^?ï.nEª?~7ì$×?'ìC®­1d?kð>&ŽWš?¼…Ó]?vGBo Pµ?ïÝtŠk~S?oè°òÀk.>ð‰Ú>ø›•ÍaϽ?q6u×Kl—?oä"Yá½?ïýÖÈ,?*=G©fI†?á:7—'Å?	¢QçŸ?2Q¤:½?'?K ×L?ïڄÏ/u?j®)ð¨—ä?Rә"Xøó?PŽf¡Póe?l1\K¶ß?e/ßr?ïœlæÄUì?gœœª/"?tð2Ê_?_aÇò"ÁÔ?|ÙY·§,Ç?_©o"QJ?ïúF×n«?@CF8>Ù¹>½Äz4£
>Â9Ì°`‡?FÕ¿7¬uZ?@@*v—(AGN3FGL J0538.8-4405@oB¨àÉÙÓÀ??Ï"èÀ5æZ¬ôÀ1À:Œáû2;?ùŸu‹ÈJ²@§9Bú?ÿ!L{ƒ®÷¿Û°.fçZ¿áÍ.õk¿á\"ÔvËu¿ã>oAGNBLL?î
ã4‡
?´o]	_>?QʞÆh}m?TÀ†G¡7?®Ãw¾œk-?´KKòž‰?ï"Q˜›dA?…âyƒåØU?dÕûýtþ?e"¢´È?…öÔ
¼n?'–—MèTã?æô¹ê‹¾S?´"är.;j?¤?"Õm,?šß|ø…)£?Ï42%…å?²ò_ôhdq?ïÑ9dêT6?LmwïÔ?%ÜdáÏ<?B'†ƒ	Õ?wµýŽôÃ?ûµœõ9?ïP}­?ªK	çÖ?Jvˆ¶àä?_|SÑ£ø?œ‹á¥?ø»?©OѲ6^ç?ïÛ#±ØL)?lé5.ÿ%ž?R±ÿëŽS?Q8P{¸?kƒûÃÎ?f®@£"Øa?èk¨>*¼?³ú:z¹Õ?£ä)8G??š™ÛEÑêp?ÉZßÑlL?²%5ûÄ?ïóÚJò?[-|ý7ù?
FŸüö?©<£5?WÃ[O.ü?ZàœÓè
AGN3FGL J0539.8+1434@gófŸê%À!B™`
Ü·À9Wßh°Ã'À;C2Öìá??ò8=-ÝÞÃ@Ìy³JDÈ@'(?7?Í02m¢à¿æ<¯ý»¾¿è­f}bT¿å«þ	rAGNfsrq?ïÕÃHÀ?{Տ <^?l5†Òq?tŽôü¡
È?]Ê
öÿÎq?fù%$bš?"<|?°;y½V?~Zޓ‹Çü?‡vîÒ:9?¡;Ëj¿??«ðxqÅD?ìTàvÅ%±?£"º/ÜÕ?ª<o cµ?˜Ðº*F?°:Ä·í|!?ž¦`ÒRÈ¥?ïsʒ_é?—ë¶ËBY?S
†#?ª ?\Ѹ뫢?l¾F¨7?Ž|" ¢s?ïì]8•GÐ?kÅ#O®E¦?X†"ƒ?cC˜ûqM?NQÕɕG?W­%¥Éƒ7?ï‡Gž"v?"#:";æÕ?hÙGÒ !Ÿ?q^؀ô¬ò?‡÷ÉÔ¦#?'(§u°Û?íÌås·²´?œ7¾>[Þ¸?£ÇڋÜŽ?• š&(y?žÓœyç°O?'ž´?ïàŠSwî›?jAÛȚc?Jí×ïªw?PšQ!s(Õ?hº6KbV?fž«è€ÑYAGN3FGL J0540.0-2837@mŸä6vÀ;@>€nOiÀ8ǵƒ+ßÀ;'j&ˆ?í…9Û÷j¹@Äo~)£@:Àß®¦Ç¿æë|ݘ™¿ëÇg©m³H¿çÔr¦™:¿ä½ÁA(AGNfsrq?ïõûHˆÙ?ƒvÚÀ"?%ó"¢Îƒ?&oŸGrù#?QJýê¹|?ƒ‹EUD?ïd©ÇÜoz?'šÞ2èÅ?p\Šê‡!b?mÜØ´:Èg?Ž§HƒÒ]?'=~EIR?î¿¥±Í9|?ŽÙ7"ʬ@?ˆksµg'?yfqвŽ?›ÕäÆ?‹bun€·?ïAŽÒAp?"À
8ìoO?f
y@è3?c'}b·µ?•€Ès?"Yÿ0ê\?ï¦*D)Ù ?¹Õ´VM-t?#G¼?~?Kÿ¢[Ÿs—?†(P
—N4?¹Õº(§¶_?ïÈòáo­H?u¹Ö›õ9?\sÛãÎÈ?V]"È­ª‡?ti˜,ٓ4?rk³y"?ïRÙ­R£?ƒº-ö.?}ÈZRØÿ.?mÖwSõ#Ç?Œe'£W½¿?½o*¥ƒ?ïÜqÀ+?nÂ[Á/'e?U3sþžy?Ip®"&©Ò?hõ1òͱ´?k=cõ05ØAGN3FGL J0540.3+2756e@f‡ÔŸ"…^¿÷þG€óšÀ7=ò¨(¨–À:"~áS?Òò"|/a©@{pkÍÙg@ŽHÀc1þ¿àÐÜ&$¿äŸ™±Ž¿ßÔ$"ï"¿ç †
 zOTHERSNR?©L©•©ä¯?§	»,ËÁÞ?™5Y½{í?¡K®½×?í¡Šžvo•?°kÒÿdÑ?¿³J=Œ?Ä©0ÙoP#?Âé[TJÁ+?µÿ
@-"#?çd²Â4˜c?Æâ8†e?ÀEÇGÛ?ª­]Ä÷ÙO?¾lDz¶Þ?ª£awóÚ?è!>uþ×-?²ÖT™?̅±\X?ºFIÃöíæ?¢ÚqQíW?—âÓK wµ?ç°ó³Ÿô?¼1 žÛøº?Àcîo'h?¹•†qÙ)?¢§ e'"?§¼´g*{?êÑuâk€¾?¿˜^¹§^²?ÏSuKö<?Ír¦Ñì
?ŧñO|Ù´?´˜I_øV?âÁ>NÍÌ?Ëù›pùK?ÎXÖZë?³o†ø}·?Ã&‡Ñù?«8¾µÎQ´?ã±VµÕu¤?¶&-Ìxy?ÔåñÃɐO?¿'ÜåÇ<?¡lp€@Ž-?ÇS›pyß?äv@N(¶?Àbôkø!OTHER3FGL J0540.4+5823@c=éÀ"š_@,'‹ Z›À9P0uєÀ;€ÍÀÓg?øsÅ@~-'Š[¹@g  ‰x¿êoœß¹¿Ü÷&o!î4¿ÙÿhI¯:Z¿Ý}õ×KñAGNbll?ïœ\U|šl?‰pÆ6'©º?~³p-°)?'Sµ]!s?seԔÄ?x{ë6°óS?îÓ[ùó?²èQ…Ö.¥?•Yr,Û9Ô?˜†jå?¤–¥Š'ß?­™Û…b°?íY‡o¸ä?¡TrnÓN?¡Aܯž?"%™•q?©ME(	Pº?›1žTi—?ëmIe_çW?©FP´'4?¥÷UjùD»?¡!æäãà^?¹š
òf?£>¯ÿ—L?ï×èy¹?u2©ú}¯?h¥´Ý¨IX?o,üR˜s•?^㤻ä?g^øÜfÈ?ïi[­¼´?–ÉÝ*ÔD.?{ÉåsÛ®?||IʟÜ	?‡ÄEdš%´?'@ʪƃ+?|ÓÄ?"X§1?'ñÜtóc?‰»æ¢œK?–Ëҙþ?_'Šý6±?îW\ðhTÊ?œ"*1?›ú%ZˆZ?‡	¢k$f<?™<UØb?'Enl—ÊaAGN3FGL J0540.5-5416@p_öŸÏ=ÀÀ?ã^è¬À9%Fí$[)À;²u®ØÅÿ?èûµÈEËß@ žæµ,@ãßbüz¿æŽ‹î'¡}¿åឤJ¿ê<:áÛÛ;¿ïÿâÖEé¼AGNfsrq?ï÷Mèé©?OÙZúÛn?7G耹oa?7Rg'¨o?G$jà4%?JI¶ñ|#q?ï\u¦5è?')™?s ˜
32?r‹{çáŠ?RJÉòy?ˆÕß,Q?î«4ÉWį?P£U?—¯µmh@å?…gU‡mˆt?'é±lƓ'?ƒÑ³$Óɔ?ït'¬JÔÃ?Œä@–O
 ?qÏ˒ä–g?r+™N™¹?‰÷o#(˜?Š-%Ȍ?ïù•©
³?Exöéƒ?3Y•©÷'?3ޚý·CU??ùäÕû??éÊ	ð{b?ï¼¹—üw?xM5ŸínJ?așà/
ö?\¼é
?x¾çŽÉvÌ?sŒáò›4ò?ï.P´½%T?€üyiI®î?Rd ~í?w9"qyÑf?…nÂԜ?t"m+æ±z?ïä¿»lu?jTäIX?SÔk²ï–§?HÉ-§²åk?aV¾1bPh?gmxj~/ÒAGN3FGL J0542.2-8737@rÅÈ _ñØÀ;Ð!`¢ØÀ:Þ$
%'À;·ª1—QÁ¿ò×øyùÁ"@LpjKM[@OÄÀ
÷¿ì|_ã{¡¿Å£/ð]¡¿Ê'Õލ¿çô%g~ÐAGNbcu?ïû,ËSê¨?7â¡ÎÔ'š?0Å~›sd?,Ž£RÊ7$?5Ô£f?0 Á5Y¥Ù?ïg.÷—Ü?'?CŽr?q¦¬¸Ác?veÐR·»?«nὨJ?Œ»»Ö¦–?ï,ò4mù`?ƒõ§s	T˜?ƒ%r¥z?p˜c^Ø&??Ï-3ƪ??~Wïܘ†?ïw¬w?ƒÑ˹ Mu?DïoÈO?M÷õVƽ?w&4ïŒE?ƒ'""â?ïýYí‡,…?(;•Ü©ß´?›§žÆX4?‰¼Ë6È?*"R-›¦&?!»ÖÇ­Â0?ïÐÙ¼çÀ?rJ'
Kõy?Yݧº?V' };{"?q¸(4+s?mF4™ÇG?ïS.r§?k§šø$?tñÁ²?`Â¥Ýñ̄?|Ž½]D.þ?b¡‰,x?ïÞ¼'–ŒŽ?b€[.uÆm?*ê\˜ë½?.øçOŠwØ?o"×€kˆ'?b	2S›OÖAGN3FGL J0542.5-0907c@j¬ú D®†À3j矶êÀ9'ï,»À;
I"®P
?ð…««iûœ@£">‹«ð@Š1€€˜í¿æÌî¹9P¿ævx{Ö~ì¿é_}¹
Åx¿ïýÀ~FDAGNbcu)?ìôËÍIt?³µlón?­8c=¤ì­?«]›ÜQë~?£zìfbc?¥cëOÙW?ä"dR²Kä?ÈÀ_ðí?Ç-QB£ú­?½–Á;ãʯ?ÆÁr'ÕÁ?ÂUÌc?çèG#wuÐ?µrv[QX?»'"·ÓI?¦œ	›$Ø?–qìš?°ÊØ]:û?ÙÏᗊ ?±Ê÷±¦ ~?Ò)é.='A?²;mDã'?Ô÷ð*äŸ?°(¯ ¿h5?î¼^¶Õо? Ñ«
³¡Ó?›¦þ«c"?š
›=†»?‰œTAe?_äâ°Hd?é|ùjË·?À?\â.3?¼)TÄõµF?±^dQrÀ:?·ö"oEùƒ?³á¸B™[?ëõÓ3nA|?¨ö¯S¨K?­i¼œ¨í ?™¢rŸôkf?±œˆƒWÍ?¢¢8uM›%?ä+ll¼c?ªn­Q®_?Êj¬Wr"×?§ï»ßö'q?Äç¡m<?¡Ôù*ɎFAGN3FGL J0543.9-5531@px+àXšÌÀ?z⟜èÙÀ8œûºöásÀ;bƒ'Öß?Æ{Jï<ŽQ@õ
j?üF·2»?ê¬ï^ñ¿ÕˆÔC¨e(¿Û̓݉w¿Í´˜õ&"AGNbll?ïôÊUµOi?Pü‹H¡n?0]Ž¡¸šu?/pdÑ?RSðÞ*?Oo5\Rû?ï]k¾?j?˜3Áq¦–?px‰Ù§•?~×¾LOå?4e¿Û«?"¯ácð…Þ?î}3hð?–ÄÒ¨:
›?‹ ã¬5ž5?í·ØçÇ?¡fƒåϾt?"²Uÿú~?ìPH

} ?ªÇ17Šœ?fë3ué]G?fœ÷¬O¹?¼Æf"œ?ª¤_¶Âöê?ïùmB£"?E<ÐþÉa
?,ÕQøeÎ?*†Ôø[/?DÀõð.ì?A-¡'WãÌ?ïÅËVÓ]?€GK.Ù²?[O">ìäj?X'˜ãö?vFž6l¼¬?|òm÷þt}?ïX!=¬!Ë?‡¸'7ß1­?}tŽ*Ñ>?qÒá^J?‹=ipp¦<?…A
¯?îé3½Ç¡??ŠJSx\Žõ?VlCîiò?Fê3é'? ¹b(š?Š$~ýpŠ€AGN3FGL J0550.6-3217@m²€ÿÚ@SÀ:'q_¾¬yÀ:?¢óµnâÀ;›ÔÓ+‹Ÿ¿ä¶Î'¾À@
ØG)_J?ùÖg?Õ-¿èJÙºñØö¿ÕÓòr›x?Â_9è?U<¿à$ÿ³ÿÌTAGNbll?ïûŸY?>hh
¥É?''Ðþ´?LmNÊ??<ý–^	9Å?<µ­½?ïƒB¡¡a?‰+ø¨ß	?lNSÀ´u?nÌîŸ?ˆ$ši"Xp?"Þj(>˜?ï9¡c"Ë?€Ä™Ó X?'#ñ®Ñâ¨?qZ
ä®c«?–¦Rz?w"öÅÞ?ïy?Îeíß?ˆZynd?%L{àÝ÷»?7h`Cé
.?­m4V‹â?ˆ9¦h)Í?ïý~‰%‹³?,ѧ<9£O?
ÚQH¹ù3?T<‹ðÌ&?0Pleï'?*Ÿ¸÷h»Û?ïÙi+h•?nR*°0?T'Ó~ü
+?Sל²ÉX‰?lMëK5.?f•gl¹?ï˜u¯Úx²?s~"³i
?uª-ŒgnZ?iåÅЄìQ?~únNôÑ?i°ß"XE?ïàVTÓõi?`í(£<y'?"RÓa9t?`"˜BQG?n‰5á÷Ëæ?`œ˜4é'AGN3FGL J0553.5-2036@l8rŸYÌûÀ5¢¡€èTÀ9¤i|›\À;‹"+ÁNê?ò"žÃO£@Œåõè¤ð?ÿÃA`r†…?ïßÉá']à¿ÒW—¡Fâ¿â:.³k¿çñ'‰ÿ?AGNbcu?îá.·+-‰? µ[#»?›ÄŸá§O?žm|ÜÔ¿¦?€+9H¥#?xÒñN>Uì?ê…Âô ?Ĝ]/þAÜ?²O/Q_Ï?³ˆdÖjñ–?¹'ÀÜ13?¾:ýŠjÀ?ëÄÿCˏ?©j^œÝ4¾?´ÌìËMyc?¤|Ið—ŠÔ?ª2)DˆJ?—'Y7Þük?å‹oÏ	¬Á?¸4RŸ¸6?ƤÀza¤?°ÓÌÊû9½?Ã./9)Ü?²Ý'1Qê?ï}h]Xíú?œí¯žŒ?‰«éÛÙä?–!4k.?n"ó5<…ì?|¯•<9W•?í[4L@}ý?´æ¾I–æ?¢•æŽmU>?¢jÏsôƒ?§¶Ô©?G÷?­tôc]«(?îSgNÔà~?˜–DVon?¡MŸ¶G?"·¾«s?'÷Ö¸Ib>?†¨r‡J?ëˆ??¥ °LÓä?·úž‰Þß¡?š0êL9?¨B꽁?ŸÇz-DfAGN3FGL J0554.1+3104@fc£ –x}@cý@,À8Çy*ŽIÀ;H5Ċß@ã®:»h@…'.¼!?ú[L¬Öã&?ïã'é9P?¿ß¾W˜\¤¿è¾ÈZÕ¿ïþÊ:Ì.ÂPSRPSR?¥øå8çB¾?ª,ê·Ìé?î'¶ÿáD?¯ƒûÈnác?Ž.êû%?™ Ü S?a³½¸Vü?mUª‡¿±?èö%C0R?ÀP;$ªk?Ëá,#ä$œ?ÀJéä›Ü¦?Á>ëèé/?ª]×U¼ð?ç^›õЍ]?°2àõE3]?ÁG">ú¢Ú?©B:â$?wø2vâÅ?"ív¹»e+?짇ïUÁ[?°¹æŠó?³eÂx´<u?«à¢1´?¥úò^E?©³³'@:?îTÜ`òÝ?­ÅÍ+ÑÆÛ?'ÝÈü?˜oÍàvŒt?~Ð=яÐ?‹sÀ?kgç?é]#½?¸"{ñö¤x?ɔòý1?·èsé©è?Âd™‹?¨UÚC7J?çÀÍÒ2?®ý#Ø|wX?½0d%2X\?¦,haêàò?´+/Íã[? R4cŸ+?ëŽü#ÉÖ?¨¾ZÔmó&?®¹Þ)2×­?ž¿,økPSR3FGL J0556.0-4353@oP`=WyÀ<®€±kGÀ9÷ªlO´sÀ;Ê/§î¿ÔaÀê–aV@'…€Þ@œ¸?wT¿Ä»Y¿±RÀ¿àšçg¿è•:í;Ø¿Ô|ÏMIx´AGNbll?ïÙ×u®i?oúM-AA?^l5–…õ?aÊÆÀÕï?fòoJ§?f_#þ—2'?ï_¼EÀÿd?•G0$¼Ì?qn®—)=@?€,áۊÔR?Y—=LP`?'Ì)Pë±¾?îyC Í;C?'TuÀNù³?—t¶²ÅiË?‡LÏ͙a¢?™bå:reÐ?"ÇwÞhî?ïpp!óg?;oMÝÜÔ?\7a»èÁ?^cBu'e?šiމñW‡?î¯7Êùa?ïôïIó?VŒjç<€2?B^q' ùÕ?HĨBš˜Ü?MmÑHY¾Ü?KŒY9\?ïҔàªØº?oÝcƒÂ¶?X>h-°!?S¡1,óÈ?p¦
[	?j½¨d-Ù?ïR¸]`×?o©õÌ?ˆG¹6žËÓ?{—(Ñ´€ä?ƒ
/ß´M?h­ uú'»?ïÙfF8§?j
Âég?7ÉYþ¬F?0X\J8	?qÐG5µ¢Æ?i1*笙sAGN3FGL J0558.1-3838@n›Í߆ã´À:jÓ_ŽÀ9˜Q`Dä6À;–Å×Eî¿õq»v¹è@
ÞM'Ðÿ?ÿ]É^Ù)R?֋Áýïb,¿ç"	.Ia¿ÍîÉÄ&,‡¿Ú¯‰¿u»AGNbll?崙ýûx?¢'(sŸ?Ožù«öx?Gç-¨kÀ?" Ÿ8A;?€¨DèŸ^¨?ïtæyq0?^¢6qO?mv{×Ë?obcßçÉ`?‹…Ãô˜
&?Œ‡(HX?í¼:ZÍ?šOàҎ
ç?•Ac?ôšÎ~"?©µ9«nï|?•+†X®ž¸?îaºh­N¾?ŸX³qó=?5ೳٗå?:ÈHÞƧ?©¸˜Ç<Y?ŸojSØZ¥?ïÖrë"óÅ?y,.	½=ð?EŠèÚ?@¡—º'v?r6š/9~?x¡þ`ü@Ä?ï϶½}	Ò?w­`Sa?Yj¸Y?ZtÃz)n?qãF®1£ˆ?rðŠŸ]?ï0ê¹ÐNj?€É"ZXò¦?"ÝçpIæ"?s‹kp ØÑ?Žçj¢~ã?võH@´n¾?笠†ÞH?xdt¥?¯Šâ1ß'?¬ytï?…Ö]k0Ÿ?xOJFö¹AGN3FGL J0558.6-7459@qáxÿûÎBÀ=‰ô?Ø]$À9´}C"À;¦üÙÚÒI?⦿aKÁÂ@A<4
Π@oß|&í?íh°HtÛ¿à2‹üU¯¿âda
~U"¿àoŸ"I<yAGNbll?ïãR9!£ƒ?a':fð…R?VRB,tL?SUÅßÅ?a"¦
×?VI›XLNŽ?îæ#zÀ?·T»þè5°?'|!"ÂwÜ?¡Ú¾Up?¥c†gV´?²·
¿M‹¹?î±xW"u?ŒŸ—Z[2"?'¤á6ÁQ&?€‰)¢¤Næ?˜,ëUŠ1?'V^¼
ê?鲒ê'üs?²åæ¥A¾?¦ƒb¿uÒ?ž)ƒU6G£?Ôۨ́<?±Üá"E+?ïöƒŠ[í?JØìðß-a?<ùՄÊϓ??9ȾjGh?Gw‡nË?=•!y¸œ8?ï[èad?ž*·efÉÿ?{7Ú
š²!?ˆ:^B"Ü?‹ Xí°[Î?–³åqÊ¢Å?ïz§Ñô1ž?s‹»Ôz[?}ê}¯|³›?i´ä¥½Þ'?'`̹û?j¶"²ûŸ?î=`‰5Pø?˜}5@-|?'H££VÞh?lw¶¾˜?£…¥žoB?•£`¬ZjAGN3FGL J0600.9-3943@nź@Ù$À:*Ÿd´µÀ9½
S¥™'À;zòÙ¦Ïã?É÷ù"•ø@g
}†@|­à#¿èHÛúDݳ¿ë»^säåY¿ëÖG¬*ڎ¿ïÿñY/WAGNfsrq?ïg_zŽçd?Ž:3ʶ0Ï?rÅýÁ/Œj?{2Jv
G?ŒÅ"tÏ(Õ?†ùfƒù?êKå}=?ÂÍÖ]Ö['?±Û~Œ&ë?³'€¤ì?»ÅXöL‰,?¼wdTW4?ìù§©Û9?¢˜aAÓ?¯kHÛ2"?–plwî?¯E«¥Þ?—Kû&˜Ô?ãwۗ§Z?²Ë4ÃÂg7?ÃëîZçV?¯¦"N-àc?Î4£F|ÍA?°…ñ}í?ï¤v–à,?…Mѝ²|?m-‹{a0Û?xÏp|¨Ø?e~ᑽÉ?|ð±êÜtæ?îÄ}%£0?°V'>ù"i?š
j½1P?¡NÒ_®T?¡]Ñ Ùð?¥¾ˆ‹[;±?î…fÜ­ë?áw:ná?¡KU"­g?…æoåé\?™¸©E¯Ð?ƒyfÙµáÌ?뵒ll?œ­ú œF?ª'~9ýä?'Œy&…Æk?µ?è_Ó¹Ì?—xږu3AGN3FGL J0601.0+3837@e§# –x}@"ÿŸÝÖ_À9ê+ùƒ=À;yóÐFÕ¿ÝÏàü7Q.@	9ùl?þ<ԟT±?²ût;Lm}¿än¯ñæ ¿ÆƄÜü£]¿àݺ¼$âAGNbll?ï6Nú»?Á©ãP¸M?_ Â>ê§?]ðþír¿ÿ?ŒPh ›n?÷JcvS?í'ô+?¸$ë$Xß?ˆŒ†bdŒ?ŽP?³t63?°ëÎ&H|?¶& •Tn?í¶¤û³¦F?œÍzÑë5<?•Ä3dö?ƒž'?Vy?ªÎ*79'?—Ô²c-æ‡?ìJ4~â´?£ì©HÿœZ?m"~¦õßØ?i4'0d܂?¼Á¸#Àœ?£'ùt#'?ï؁;Sé?tæe!ßM?Ii/¨ý‡ã?D|xF)?p'<}ë°k?s5ó»¦Å3?ïJìÓ?žÖ2["Ñ…?qJŽpP?tD/Gp?'kå{øÒ?šÝü#+?ï)3û…	?ƒ†õE4e?"&9:_R›?r–ØËeõú?Æcö b‰?~å·ôàQŽ?îô<÷ÆåF?…8™sM?bJ˜Ð@?Q‰Ðš×ó?Ÿ7—µ­5?"†–¡[s³AGN3FGL J0601.2-7036@q­••À=Ÿ½@gÏÀ82ñc…
–À;]íCdٞ?ú#«kS51@º°Í@6ß"óŽ¿Ý-¯iBA¿æ!O$Í·%¿å0Ûrµˆ¿ç®(^P'AGNfsrq?ïôÿ¤n‰?Je¶Àb:?:ò0ãmB?5üWMÿM?Nöõ6m»G?D¯¨0^*?ïƒ[Q®?‹í>1¶S?kwŒ…	?tê©Ç8g?ˆKUWºþ?…`ñ}þ€?îk:¥\4?Ÿ›ªLŸ°?¡Aœˆ³Ú?–jKÎ4«Ù?š{y"Iº?'SÁÊÅt?ïÀüéŽé+?'ɐ
‹M?M××TŒ?b3÷H_a?{ƐNízú?ÐZ…cø?ïùã-·HV?<Þâë·×â?7ÁÚPO?3c$T¿Ñ?9$¸{'+ä?.,L°œ0–?ï҉mã™~?q+;"?
'?Xx˜
™˜Ý?V5³únŸ´?p#‹J¢?iò3ˆ |?î¬þ€£ÿN?š¥Õ[†>?šÛœ£9é?•Eiâ3ö®?	'´Œ•?Š.C¤w7?ïò¾ÁqNø?`:ޒbê?=Ã8:\?;é­äÚu?SXýiò?\øm_zAGN3FGL J0602.2+5314@d~`Ï6@-,}C"À9Ñêä±À;£¾:bÒ]À©ƒæTi@«¼pP±@Du߀-¸¿í'>9²ºc¿Ã¬Ò['¿Ø ÈýµLþ¿á<$§cvAGNbcu?ï÷æ—ë–?Iî…Ë÷G?4âTÜ/?ž?0Lïîã?Eôxʃ|»?E©¹Èø?ïZñëÀ-?œeWÊK¦?p'g¨ú˜?m8S,ô'ú?™áꠅ7?›²Õæã
?îÓ¹bY2ï?'Œï‡ÏÒ?ƒ±¯°G^ ?sd«¿£¦Þ?›¯ûÝeß?'ÎQnþ?ïºð#ò?xÍ÷Á&²?à—A<É?%7ãdÊu&?5ÒIŒZ?x¢ï{qê?ïüôúµµ¦?.Ã3FgÒ?"‡ÁU/?ä
͵ô)?..Ññ¸?(þÎAáò?ïΐoµ€¼?€W)Ú\hõ?ZX¶¢®^)?\N§x3&?r!šÂW?}X.K1m?ïtR؅ú?ƒmÌxŸg$?vjè·Dæ?fA2IÞ+S?‡¶;ó!?'ÇìKkÛë?ïñ å0yx?Q)è^á%a>ð»ç¥Ï>úÒpN¾!?]{EÛ]?Qñ~¢ƒAGN3FGL J0602.8-4016@nÜ"ÿ‰;À9ó¡_`¸§À9#¾ôœõoÀ;V»ºUÑÄ?ä¾*ós«@=
¬æÓ^?þÄ6á=¿´
'½'¥½¿ÝyKyÓÍ¿Ê¿±})æ¿ã±þG÷™AGNbcu?ïåýƝf?jP¯Á:?ZÑ£ìàµ?cˆ@ø¸ùß?[`ÖeB?W<$fÆAp?î(ì~ Ÿæ?­÷œ ˆkâ?'Îë3_ëÝ?"-į(s?¤	…ýÙ«?©§Áœ	cì?î§ÞD³'#?sBÇÚv?"&Ë1Fgü?…0ñEšAt?–Ýl8T³ ?''—r$)?é®z©`ÙV?©8ácè?•V¢'ÖJ¿?(©"•Ú‡?ƛA!ÑP?¨ØZUkT?ïòSx¼Ä?Sф<ŽÚ?J5`{øi?GÚPÞ´¿±?L|¼ò—À.?E ÝÙ'±?ïLAM8~2?–ýúÕ]è?}‡ä'–η?yXþïí·Ì?Ž+º—5Ô2?"+* ¼?ï^t×ç?î®õ?…l•È·?zRà[w°s?'ó"AÝ\?h×ù‡)¬?íŽiøl7â?'ч>¸…?"áöVhTn?zû^?¬¨eOÀ%­?ŽCú,‹·AGN3FGL J0603.8+2155@g"	Å!Þ?s\žà*­À9dûy‰À:þËåF@V¿þ€v²äÄ:@ɦ$Š±@βÿœ,ò¿Ý±ÙH}"£¿åö>
3¿áª<Üv°X¿ÚõÓS'pAGNbcu?ïªrC?¢<»È±?@@êw²l ?GÞUÃè`?œh·#˜5–?¡íæeä±&?Ö‹e¤I¡?Ö£'17§Ù?¡Ø£©>²€?£d/–¥Ü9?ãá°ú%?Ö£™L¦?ëÓ×/Û?©á$=d?˜A앇??ˆô"²ˆ?»\÷t7¬·?§»Ów®.É?ïµ	¢>+?|yžÈÉ°'>ÙpU°V`ç>âOzNÄ¥·?'ºi}ßD?|x~9it¸?ï²|)¤Ç©?*n⍈§?AùðÒFà?Pp3È?'AV~À9?Üï×)LI?ÞL?QW?ÙEÌQkœJ?¦N<›^7?¥½ÛäC–?ߺë£Òƒ?ה¸OMN?îsŠ§@ÿ­?—b|áÛ?ˆ°»ù*?}iÍ)7§?¢£i\Rä?•óZp²ò?ïîaøÌ¼?T<±ðÖ&ö>ÂHí,Qޚ>Ë?a™u-½Ì)?T:0:ÍáÁMIXED3FGL J0604.1-4817@oö:à;>šÀ;€¦@q	XÀ:O
ª}ílÀ;¤Wèõ!€¿€‹G†¦F¬@5~ßÙïË?÷J` |!¿ï½Þÿ¦L?ïCy^]$ì?áMó½ÉÇ?˜–Œ°¹,AGNbll?ïϪrYä£?þ5" \]?.Mâ–\7Ê?(ãIŒ/Ç'?w8WÜ7z?¾H%B@?ïÝLÃÊ?‡Lp(Ù~f?g?Lôµ×
?hcT)=Ò?†8äõxíœ?ƒ£}}l,ó?î"íI¼Y?'ô17'?Œéj:§ü?ƒ:]mÊ+?ží¡°HŇ?à_¦®ªù?ïÂím7Î?†vz4êç?&tc Šèš?8f 4–í[?}Õ¦".¢,?†N×ÁñÛ?ïÔ©úh?€=k —¥?.ˆSEÏq«?=ö,')"?t·:Ö ú!?€05IZ^?ï×*ž0¤…?p8XÅs?U`
'x¨?RÓêQݸ@?n%\'žné?iéF©ªW[?ï! Ž!ã¢?µ$øM}8?…'¯'éÒ
?ƒwM‰^¯¬?'r΢½?‰5P-¼=?ïô-á‡w?WOÉEsœ™?$,/‡?"Ç
Ì@'Ç?U·bƶk?V0^(<§¬AGN3FGL J0604.7-4849@pã_€™À;€¹ Gž$À:T>iƒQÀ;ÅûqûÅß?¶Pf"ÀŽ@×_´Æq@0bŸ²bh¿á7ÈK]Ìd¿í|jŽ‹•í¿~ŒË*
j'¿é܈¬ŒeAGNbcu?ïÁQ՛ä‰?Ӗ؃– ?Lš£Â­Þ!?M흌&?{ÃÀ³0½ç?~^ºÎ-,+?îœøèDޓ?¤ç¡9v?Š>ÝŽ:?ŽEAo&?ŸYCƒ±|š?žüm×Òlý?í)ÄÕ1 6?›oÍÈiH–?šBOè/
?†Ùéu6ÿ?°!Eg®´
?–«¬é/?í8Ö ,¨!?ªK˔ð:Ü?}t?îsÌ?…̏«¨;¨?´b
{ú?¨ˆÛ$µ^?ïçdØòŸð?cÍ{Rď?5•ø')?3×Ðӏ#_?eé$Tq¿?aøÆÁk(?ï'ö ìÛF?ƒ(BÁª¥?rF\_™D?kE&VR0r?'_)'"Òh?}Ö#òeõ?îá'Uè ?ˆtľ"ŒL?†ë"ÖCë~?w  …X[l?˜Wër8?"¦È¡ÜîŠ?ïL½Ü!²
?‡)épbå?w~'ã`!Õ?q[uc-È¢?ˆŸ¾z8P?'Óp	½@AGN3FGL J0605.0+3756@eƪŽ:Á@ü.ŸûˆwÀ9³¤™_¸À;®yð'Î?û¾æ‡^@
|€È'Uƒ?ðü—x,6•?ïõ»tpüS¿ÔÙ3î"¼¿åª§Ç|¿ïp<"
œ(PSRPSR?oü'i'ž?qw7Uìð?íÁ¹¦Th?¶•ƒ	ø5ã?°òNA7 ?¶96Èu†?‡!ü"´´D?¯kþy'=?ê"É]4d?Â^Ô
€=Ÿ?Ä>»á†Üí?ÀúI¹Ê]?ª¥N_ú?˜Dh¢¨?êD—/m<*?°…BŠï&?ÀDO»)6Z?¬ä;Ñœ?©Fºê?Õ? ̛@ç?ìLÙÄF?°Ó0Ç8²P?°ü‰¥ßä?¨E2@gé?~:úÀ6¤Ÿ?‹˜™fo?ísÕøo'à?¸/¡QG?²} j7?¶¬½G;?"ÂWSAÿ? ÝÍi¶?ê%© €q2?¾k5\r
£?Äñ	"¸À7?¼Å6ø±ú[?¿ŽË[æ'?ª;Ž.Sø?è/7}<87?².Ï{qÉ?¾÷x»W¶?¨îÍõä´?ÂBOÁða?¦¡FÊæ?éȉ»Ím~?­B½Äd?«Z[±Ÿ?¡'ïÒ1ÒPSR3FGL J0606.4-4729@oܱßv½À:÷ûÀÖ…À:üLû[À;ƐY~÷W?Çû¿¥-1Î@Ë|½ë³m@žšÀ
F«¿ìœ­¹rc0¿¹"¢L×°<¿çöK¨ÂMå¿Úq84'q=AGNbcu?ïV3KdŠø?•HáÝy?÷žè?…ޝ­Fí?ˆ|'47?É–Ô›·Ò?î6	*1h?³<RüE?úé¶TŸÆ?™ÄE‡r?¥ ²ñ$Ú?¯‰b%Z?ìÄ÷B[ù? üè*m´0?£,v§7x#?'iÁóQ‡6?°BQu}+?™aºÅ?ìvÆö¹?©´9薲?£ûïæ\Š? {Ò֏	?²Ê…ŠCt?¤£Åù³?ïÔ&òqø?x5¦˜:H?a¤tÄ'±?l:ôl~Ñh?j4™Orà?l‡3¤Àé¾?ïy",í@W?˜¡\|Dـ?tÇ<"0¡ì?"VÙ0€vî?‡;VŠ~³4?'Û ªMÿ?îÞôkœ?‡¬‹ÖæÀº?˜Bì³J?s€—HhE?"‰/¶sfv?{‰¯0¤¡?ï5–¡†fÑ?ƒ–ò
2Ÿ?{í¾_MÐ?tšLÍY)?4òÃ.þ?}ºëž« AGN3FGL J0607.4+4739@d´xÀ>-@)ºžEÑÀ8E&s1PÀ;?uQ»´wÀ¥Ç¥EŸG@[sºÿé@.>`7ù¿äåÉkvú¿à\¬‡n/¿ßs"¦1Fc¿äª¯¶¼j)AGNbll?諭hõ§?ƒ
ÐÎf6?e/äáö?b,˜SDd?€14ZÌ?€L<Y¥ R?îcã"0ñ\?º´¿œ¯ðë?{÷`p|o?"MĆ.?¦BÚ²Gù.?¹Â¾œ¼?í_"›?¢~£àI @?™	5Úoú?‹Q–¼ˆÝ?­ƒm.íÙV?ž‹[&y˜?î|
êEÐç?¦¡¨ï*£?M¤ÚÅ6{²?pþͽšû#?§Èï^ ‰?¦I']žÓ?ïêع?&\?e
Þ°ê	?Ké•ü®Þ×?H«˜¿?\Yžá?`åÖ¶Ý?ï°·Ybœ?H㮧'?fÛ¸.Ñjé?wi‰¨ØZ?|6wTX†?†ß,¤7}?îüÔ?:†?'kª*Ýå?†O®Zé'?€éÈjñE?•=¯ÁÈ ?Œz7å°¯œ?ï¦LüVÓ?" f{;¡>ûB"\Í0?	€/áé‰~?†_Zd—²£?"—¹"SšAGN3FGL J0608.0-0835@jø€àe0À+>~ÀÐ?À8VÆ;¹²À;£NNA¬?äQ·
%‹@i°Ü+dˆ@û>_a9¿ÞÈc¬!Üt¿æêðü××m¿äŒñÍ'¿çŸ°·ìÏAGNfsrq?ïø§.‹6]?AŸ Þªø?8Ïã°qÎ?4'†à£-ö?AV݃L6‡?7ûÔSêR?ïOYE°R2?•·ŒÎÎèX?užãƒV?{ôsDô8e?­PØ A?'7ã\V#?îѓ˜Î˜?Š^Àuà1?;Yîì?{€C9—!®?—0>]L¦?'" ÿ`8?îÝÈòlL?'òÇÐgÅ?d<1Q6I'?`—û¸!4? ßºì̤?'€ˆ¹h5?ïü™W™2Û?1ŽêVÞþ?)«=
ö~?$š)4hB?-cØ©A±?$õʉm}?ﺋL'm6?'•_Ѓ'I?_°tnÀ;À?]˜Ù؇kÉ?zÎ<œ:9?€¢ìÝ?êÅ?t"^fÍy?yç¦Þ¡ÄŠ?htŒÅé?'£±ãî7?jnuÔö˜?ï´XÖZë?s~½ÇA?Râß*>å:?D2³w§Ìê?€œMõG'€?rÍfÁ AGN3FGL J0608.1-1522@kÄUŸnÅ°À0cZ _†xÀ8'™" äÀ;`l,yÏ?÷•<ÀO»Õ@O?'¡Û]@‡Xöç(¿â=³œÐæ¿ç±ë~$|¿ê±¥?s¿èKÎxژyAGNfsrq@?ïêížq{?Z"·56?Y°ßü•jr?T,ÜJ¤Ú?PsãÌHŽ?Hj$i6?ï.n9»ÚÙ?š¶F$[çÎ?z!ŠRJ˜ß?{)´7_QÇ?"©Ö8ím'?—bÜJš8?î¾ðÑÂ]'?'ök~>¤t?½mféK¼?ƒ'X `?—dx`Ë.?‰°ì"h©?laý÷?/Lxói–?†JLWÜÚ?…ˆ"vÜP?žç,GÒ>¶?šŽmê´×G?ï÷üÂ?¢?E},°Û'?C'ã…,õ?AP*€›°?8õMò…?1U^¥úÏ?ﱄã1ƪ?"XÛ=ôÇY?d¤þ"¢–d?b:â²òÆ?|ë«7¹?3¢œà‹?ï9®6Ü?†k€deñ|?‡Ô@¥Þk?zt®'š?‰À1ÈtÚe?~¿øâU#a?沈ùÖµ?€æP³†[?s»9Ç·è!?iùŠ4<ù?y»lÊ{Q?{,¯¡pæAGN3FGL J0609.3+2131@g£? §??íÀ &jgÀ8Ӟ÷§kêÀ:Ý12I(?ýSj-E]'@
géÝSؚ?ûè!¼é*¿àñqÇÿàå»,]¿ìK¤™'¿ëz¡5¼œËPSRpsr?d¸훬H?hz"}ÉW?è¯5²¿Zs?ÇE)WM€?ÌðHÁ©œá?Ç+Ñ	u}?pçþÎy?€u[®ràÅ?àe"ŽÂ?ÅÑOË;Ê~?Þò;¿§Ró?ÅÖ@HÅk¯?¹àۀ!
?¥ÕÙóž?=?åÀT냊þ?³å\݅ê?Ì>'á?±QÍ1÷sê?¦	lAÉX?œëï\+À?ç\A*5D?¾Gñy]º?Í¶œ´¬?»ã¡z?i«.jAÈ?r¦ž†† ý?é?ë2="á?ÈGvÁÓI"?ʙ¦|"‡·?È žlMlV? ÕZT'?±Èr§.?ᴏ´h|ì?Á"ýØ"?Ú|5FDD?Á?/–VÕ?ÎóÝ}8Ð?±A‡&'ñ†?âœÂܑ™y?´Éÿt:–?ƙ›aN?©ñ†m&zç?±ÿ±*ÎÃo?›Ô`|Ýð7?èrÏÖA•¢?°Æý×#m?Å4è;B?¬sgPSR3FGL J0609.4-0248@jT&Þüz:À%AŒ 4RîÀ96ÕVß	æÀ;:"Ž½ž?Ñr†]…Iß@M>A©™?þ_O€ñ­¿àWƒ@€'{¿Ý¬)AusÓ¿ÝÙ«‰þhs¿×À›
–AGNbll?ï¢yÞØ÷?ƒðÊC_Å?b°ÁêHÆ1?`"`àð,?'µWÐÍh£?N‹e8½Û?îxŽu_cÏ?­ˆ"˜æ²?€Æ"3UíÈ?€m«³^¢?¤EwœX` ?ªsJwãàf?î84¡"²!?•"{Éš?"±¼%?'jx¸±3€?¢$'ŠZ!å?'*°šÌ{l?ìÍP{v ¡?œÞ¿æƒ?r²†å¶Íb?pM­òûC?¸jSµ"¥á?›qô7j'?ïáßu	Ü?gP@`HC?O¯1žù?Lóíä`U%?f4ɃýÃ?c<
eƒé_?ï|uð®9 ?'½¤ž÷?lNà¿òQ?n‡¡ðæ<¡?‰ÎËÞ\?EÝÄf­Ñ?ïNþp¼^H?ƒ5'C¬Þ?ƒ#L
oš˜?v¬qŠS<?‰¿™›c?{Ã5†4?ï'¬ÝŒ?€Ÿmaèµ?hNícœ7Ô?UÞWÞi$'?œ£ì³æڒ?ӝÏÈÐuAGN3FGL J0610.2-2059@lwXf€À2-ПÀ$HÀ90¾£%4À;	Ü!Ôf?óûíÖ]@q-­ã(@°}_|<g¿ày·ÜBx¿âB¨ïM¿èvN—×fs¿ìŒ»[•ÄPSRPSR?­Ãêu?­=m©é­_?ìWüÍÆ?¸žèñ˜Ÿ?¬½Ž€?¯J[— /°?©óª˜U²ö?²¢°&¢?èVq+ÄÝs?Á÷BÀ"?È)Pª×w?¿´Ì¥àz?תX1V?´°@þψ§?ݜ²ø\{?¶EUjé ?ƍG"^ä^?ª>"=DŒª?¼Wo—Vb?¦þ1$¹i?èHŸôt?³"à·»B·?À×<1´'ÿ?ªÞö^ÛF|?¿ìÚ;þ¼g?¼OŒ€èƒô?êâR3î?ÁhÍqÀë ?®~Md—M?¨dzù§h"?·;Öoã¾?¶È<`Ï#?å•{ICã&?Àg«nòë´?Æò×€ª?ºc܀@y?äJ^6ÛÎ?±¡gbµÞ?Ðý-Fxú?®~q{ì€?¹¸Y/=§£? [&Ší?ÔY\ÒÙ¹?­v]
#?â»%Kz8?°k[YŠ8g?¸Áb]¿—?žÃ†âc¶)MIXED3FGL J0610.6+1728@h" ³Ô®¿èbšë±À8ÓÿgSÌ0À:ò+ÐÂü?üEy Ó4E@Êê?«ç?þ,Mìm¿ÏnA§V¿è神ç3¿ëؒ2>¿ãl¾U¼OTHERspp?Ñ"ÍÿkŸ?Åh§ðZ¬°?Û'È=hc?ÏWQ[În?ÓÏÕiÃ+þ?Ç³FÛ¼?—"Æm"Š?¡ímVD°3?ÈáÔ0n\Õ?¿­,Í­6H?éFM°ü¦?À÷(œgn?ß\çÑNÖ?´€í‡I¹F?Ï|(M.º†?±Ð «'?Ñ*Žñ—Sæ?³:äú¸dØ?͒ãM}ó\?º‰Øö³…?סÐÜô.³?ÉþþßTË?ٔ½{9öá?¸1e¹Ô^?áAƊy§G?͂Ž/Wÿ?Ò1÷ÂLsÕ?Ê:¦ãM(?ƔöS¦<¸?¿")"ªÊÍ?°	ªSÊ.A?´±¾øIù?ËU!£?¿<cóðR8?ç)'LmcR?Å=f],+?㏯FÃ͏?´É½þYµõ?˃¬ZÄû%?°[SÒ?Æ=–Š+Ρ?­¨ñ~ǁ?×!€"Zÿ;?ºEàõMÊc?Û)È":‰á?Àêw¤ôŽ?Ëin°¯,J?±ö>þúdMIXED3FGL J0611.1-6100@pá´™=SÀ<O <¶jÀ9‹€ì#ªÀ;Ó\9¼º0¿þÝ3Tk<9@ˆy½0M@£Z?¼ƒ~¿é\ºO5Œ¿æ¸Á¤>}¿é`Osä0õ¿Ú•"»T7AGNfsrq?ïüšÚ%>Ã?4#·G`Ü?$ªî¦ƒùå?&æՊk?0Ó¸G—óQ?*õ­cºÐ¿?ï–Æm.£ú?"eί†±?f¨p³"™Þ?h0´;#Ï?"¤Hö{!?EÕ3µ?ïN,;zÞ?'ÏùÖî?…¦ú#sØ?t2uêá/?"g^"L?{Êd@à?ïÖÐB'ä³?q€Õü—ô?ë+Št?"ÊѶ¡;?thB'ÎY?qrõ—¦9?ïýÐɽ?/‰eûšÖT?à%›rÚ?a—}¦Ø±?'²°.֛¬?&IäS¿Ù>?ïÛ:ZB?kQèmвœ?R²q€¿?PÁµƺ/?kl»'>º?f7Ò͕f.?3‹ƒè?uNòÛ=?x!Sëš,c?pV[çgnØ?~™W'Û\?i†'5äÖ?ïùôp³O?G¢IǼ">ёóJ	Q>Ö]Cæ[?Hñܞ¼?G
bãZ¥ÁAGN3FGL J0611.2+4323@e;R`õä@' ^YQ«À9Þî<³åÀ;¤ÏFúT?ÕL¯/æ)@´8V]°@Wé`}¿ë—&Z1ϱ¿ãn"±Ž"¿×'Œv4S‰¿Ø`|ˆAGNbcu?ï™ ?O?‡
;m>qÖ?aUg§5cç?aëÇنŽ?…b–Dœßl?"ˆû²UŒ«?îˆbX1<?¯
ô]‡?ƒ,Ž+æÞ}?'Y+ë@U[?¢¬æN9Z%?ªùhiÔb¡?íût÷½€?—Óg×»Ï`?""P¼mõu?&̀›*Ç?¦†ˆ$95Ð?"zJ@bh!?îxQ?¸§§?–",J¿IŠ?uDŒT•6;?yŠ9px\?¥ÒZ|ä‡H?"v'=ç?ïÖBŸaڑ?u±32?>ñ?Réæâšbñ?Ui€Ð‰•¢?p$6x/+?r2ÑÇ/p?ïš.¸áC¸?Š´ê`Ž?k#¢oÌ®©?jÂ>‰ÁŸô?'«i7œ(?† wÒqë?ïD‹"ëe?'û‰â6'o?'œà© Ú?w=Zv"—?Œ@:+ÃÁ?zJÕ¹Ìê%?ï¡¥ ¦?s'´v€+?j˜ƒhKŒ?YíPâ°ã²?€ð·»?pY6ÔZ¼5AGN3FGL J0611.7+2759@fõ¢Àh¡@ã:"À9«œàuöýÀ;Då1?†sðº±@.Ääv@7¹½ûN¿åÓx³£Ž™¿Ûõ>ŽŽ¬¿àÞꌃå¿îŽ'ÞQQAGNbcu?åÓÈË?Ć&'>W?Òâ)(Kb?ęV}»Â?—|êâ6–j?•¶š•ÉԖ?ém˜Ù͈¬?Åq9jÒ(N?£Î]½Ç<?¡:|fx?ÅV)NqÂ?ÃUHW˜Ô^?åémò?²Ù_³?Ωºð <?°ÇH¤?­?³c«5£Oü?™¯*¥p‹?êjÓTj)X?©ˆî¡iäÏ?£mSÉz«?•Å:ÛC?Áy]¼;ô?¦k<ÀÎÝ`?éíMBJu?Àj;jϚ?È]xûƒ2i?À…Üßz¶?Š-ú©Ø@?…;À_&K?íôØVêë?±<áæBc?ŽJlîgg?f·Ž?©ãÓ^l?¬[ælÇX¹?é"è
Ð×?¬^½AãÅ?Äv9kIw?©
¾íJ£?¥Ø˜­Âb¿?'Ùٍ•ùS?íú$ü¹¤|?WÇ̎·´?'b,†Jü?}bș?§Ü"n½?Š½"B_ðAGN3FGL J0612.8+4122@ezWà&Eå@%Ö3À7²8%
{"À:à"Xð\?çXwýVq@@¡)3!@3å?ŠY‹¿ÙíÕǃrø¿àïr«20¿à6tJ¢¿Þ5	cÎSAGNbll?ï컜›#)?aÕÙÇu?@-r¹Y??f†Lô2"?^rB·e‡?]ý{%C;(?ííà/w‰F?·6ð†T1I?–Û¼Ø"?›Ý|¦æ?¨Öô"æ?²SEx?푠éïóC?¢§°;O??'à‰Oññ$?Šhï"gS?­u¬¼woA?Ÿ43m¨•"?ê«Ó×Ô¾?©ªl7§/?Õ›tϱ?‡åÙ^Á-?ÃSaò
y?©ínáh?ïùÀÀú܀?BÀ±%þ$d?)A£0?#]LXßL?B¶,ËbÊ?@&JBï]?ïJ'ß™‹µ?¡0\œÁŸÑ?|¼©ìB?‡üEͅ?Žý3†"?™Ø®Á"?î¢!p6¹?šðj?‰¹Ÿ¬ö?…ù§=Ÿ‡j?Ÿ:õ6‡ØO?•!^M2ü?î)(™†?ôx‹x?"yéÿLL?lƒ:5q®?©aNƒÙ"?‡×êŽßAGN3FGL J0613.8-0201@jMõ¡lèÀ"—ô|ôÀ8
¤ž°ZÀ;#wÀOç@ÿ…$'@<ó%|?þ5لÁ¿¶CÛ2Qr¿ÜÜ#€Òg/¿ä°·•­ü¨¿ïJÑz kPSRPSR?j6œ&/?u;sdI(?ﰄç¨<Â?‰€fÌûŒL?z¢ƒË@£'?ƒ×J*,¤?c&¾©ö?ƒîBaO?ëç<WI=?À'¯=èk?ÀvŠ²^?¿õúîs:µ?žÇØß9<á?'5âéXn?ìF+¾ß?¤F¹½oov?¶«×:¸-?¡6²ÿÓ&²?‹éófN?ú•ä"ƒ?íËqXm? "øz_›?¬…/û×bŽ?DEù÷b?d¿m ¸/?†»ÊÁê"?ï¬óPo.6?™KÉì£?&Ê öÐÄ?ðÂïUG?ru'÷îŸj?'4¢nG»?ëïkj²%'?¹N–]ql¡?¿]KŽãv÷?¸öÖÛãMê?¨´	*¢Ë/?š±í,ъÆ?ìÒ®Á§ˆ?¤n;ˆF~ø?²§eò{œ©?Åƒ˜«{ý?Ÿø¦là?†ôz¶`—?í‹áÍ1n?™ë)?U­?§Eã'éW?"È(^#PSR3FGL J0614.1-3329@nà`þG™À5Ô´ßp=€À6ì^'À:œÆä@ý#¬¦@u˜>¥­#?þÞt§Ç¯­¿À'ª~nE¿Ö…¦|X¿áXez`Í¿êz¨Ea'žPSRPSR?"Žüg1|?©PvA?îÐ1Gí÷·?§½­ÔqÙM?'jÚ¢•?™F"îù?X_Õ7àX#?k±Øáub?íó{uŸÇå?°¢Cæ
•Ã?°¤þó'º?°n᜖í?½ß$"2LX?®<¡þ-?èPsÓÑ?·ÁDÄBI-?¿ Î/+?ª¶7Ì)v·?bÄã°I?h-'*9X?ÏSÝ?œF‹7}±?¥û3Èá.?›´ýÿŸ?Xh¿	ªI?˜Üú§È?îúXwK¢&?¥S¹¢ŽåÕ?\ˆUÊB÷?™&õÌÆ"×?jŸÈ¨¿î?zi'±:í?íÏKç›@?®kмk÷?°²7Z(MN?­"+qkÿ¸?ÅíèAX¡?¯#áúu?æ$•Fßɐ?µP£äÿ§?Á£(8®?¬d•tԐ?lфÝîà?]îæ4úI?îàG/‹Ö/?Œ]#`q¾? 9¿ñöfŸ?Š·ññ'¬PSR3FGL J0615.4-3116@mÊòŸYÌûÀ4ՙÀ0XÀ9Òâ7˜ÂÀ;ÇyÒ9À'«0ð¸º@:ÀÌäIÁ@¥@¿ ¿é_äy'¼V¿å…Â+¼¥¿á"",zåØ¿á¸]Üv…eAGNbll?ïçzDÙh?dÅò\@;?CEž€»tÖ?A'°ªˆ3
?dòI(&?bþÓ®^ã?ïƒnIFn?Û›áìp?iÜAµ†"?m1]ï2?ˆ­]GŽþ?;Ц–Å?î²S'nõ#?ÛWB"?Š	¢†\µ?u%ÖZ=ƒÜ?œ°¼Í…—J?ˆ°~
è~?ノeø`?w:§EÞ?9a :n?¬{ÿ0z?€Am'\¥œ?vòŸmŽ»Õ?ï÷Fš2	¬?K5~
NÇ?2=âŸ:µž?2d½¯D¿,?IƤô$'Q?Fϐ¹Ýš?ïÖ»¥?pÌãÄp=?UçàÎ[H?Sª>Oïs?oú¤G"?i­D^»4'?ï‡'îeE?ròþÒ½Ù?vèǂG±Ý?c5Q
֓
?'ÁՂ:óÀ?kâÔ¡YÚ?ïõ»ç;'?Nn?¥áäu>ݨÂɦ>àÑ1ଯ?U¨ß^'.>?Ne'Ã>'AGN3FGL J0617.2+5701@c­UàqÅ?@2ì_9K{À90½7-"À;"*m'ÓÒ¿úSndzÞ>@OYãÌÆ@T?b¿ÜsOa«ÛT¿ä1T>y@¿Û©NßG^õ¿ÙÛË}lg\AGNbll?ïñÍ ?÷£?V8Ð
?B܊ï?9¥¥;]Çr?S^6Xäî?RóNL	?Ùþʲ?'G˜kϺ?nnÿ,g‡d?k˜rqoS?…A	©"Ÿ?}ñi܉ü?îå…H‡`å?ý2?‡ƒUï҉›?}¤vÚ	pÌ?—«ò4Š?‹a»›qí?ïwšüÎ¥É?‡;ðÀì?!¬Sš—˜?)ÒµŽ—ùC?éGº{Qà?†ùF1Ðx!?ïøä9ÈE ?@=«UZ"Ä?:S†:ᨗ?1£%ÃÔ/ ?>ŠªÄk`?7E¨ÅcÁÉ?ïÚç#)¹?qèa—æa?X¡›ø¹ð?S«kš­×?hÈ2«Ùw?l4ÄH?ï…sŒÐÅ?yð¯®Å'?z"Y_Öøõ?p K¬&;4?svuÏNU?oú–ÁCrï?ïåÒ»µ^'?b…ÃÚõn>üôSz±>ýÚF"¹×?ió[•q¨¤?bw6\!WØAGN3FGL J0617.2+2234e@g¡ŠŸb0@E?ªºÔÀ5iL"=À9¯Õh|Á@M1;ŒH"@d³kýª?ûwohÁh¿ÏDô¦°ƒk¿á4U݂&¶¿áW35å?¿ä鯁7xOTHERSNR?¥å6LÐ?¹|Æ\í­?á	QSjòM?πÀF_>?Û0¶•—›,?Îî'cNâo?L¦¢Á®ªQ?qu_k¶?ë"ߏ`õ?¸Î"¤Æ?ÃeÞfRD?¸¾²óPÒÓ?½Ù'#0?©#lS?Ö¢•¡gnN?µµžd²ñª?àþ"´'ds?¶=ÁøÒµ?jxÛÚÀ?g•ªî ó?å©"Ö?Á²'~túÿ?ÔxÊ^èæ?Á›(?³«§'%˜?¿Ê²*ßý?á?#£¯X?Ñ^Lœsz?ؖãÔÄ©?Ñ%(E:ê?^U-q»Îµ?uSmmõ.ž?ëÏA*ß?µ¶øè ?À†Q™¶Ü?µš¨9'én?¹D>ąf?¥'Ý•VoÍ?Ù*²6Q(?³UîTIô?àBkNFxÏ?³kúÏ|p?kS¤}²b/?f)mvJì?æÂG{rDÊ?·VôÚ¥+?ÒDÉÀuGø?·^í)£aMIXED3FGL J0617.6-1717@l¨ŸÆÚEÀ.1Ïþ°t§À92éf`‡)À;PñîÅE¿ç`Úö±!Ì@­À'U'z?þú¤¾æ°#¿ä6À'«ZP¿àb
¥^ó¿Úmœ;èí¿Ï¥{ÔP"…AGNbll?ïùù9M¼?<$¾Í؏"?"³éˆ@qå?I!D
ð?Cnlsë0?8'£Éâ]ÿ?ïtáÜS}?'«c¬~¤?nLÚPOm
?pºAoÞ?‹4Rb»p‹?†š˜°1?ïI¤šY"?}a‰Q1ÔÄ?o;Æ+}?r6Œ'mÛ?Œ"jGÊÙ}?tïãÙªêó?ï8H?xª¥?"À´¦ï?''*'C'?)—>7œ–?˜Çóº›s™?"³n^H"?qsŠ¼?½Á!¢*ür?"wÛG¨¥?½ÃóVÆ­›?8Uz¼hMÐ?*Zôt.ñ?ïϨ˜KL?s:E	˜.Þ?Wû
h"í?VRÂiՅ?r,ñ[°Î?nh¾+³…Ô?ï­ôf]›Ö?hî—âZ3Å?q²&ãـ¨?dßE!?wS¦Å°?X¨üoqå?ïÑúùÊ¡?`
¢á/ ?ގ"–Ÿ?
Alh?w"ˆ/TÒx?_ù>u© ÞAGN3FGL J0618.0+7819@`õÖàL'@8Üz¿¹¾ÓÀ:ZÍcˁsÀ<ÿ¼ä?娖×@Âùó÷^@ùÏãJ=¿çÖý3¿éMb˜óμ¿Ú¨O‹1U¿â/p¹"#AGNfsrq?ï÷Wœ‡h?MýD9δ2?>yI¿DÈ?@‡åö]h?Cfý+Ka?Cö:Ënžu?ïUoʬû»?"ä"9™ƒé?'Vq'úrÚ?~¨!c©O÷?ˆM›Ë?\v?¶­ðvq¸?îêg‰bP?‹Én9'?‰*:¼—?~KÏÕ~õ?–*­ZN}?ƒqõš@"?îÈwÚúYo?•"Í暁¶?†øž}R<î?‡Ÿži­±?›tµ`Så¡?õ"p1/<?ïýFãFêS?0Ç¢ãx?%""p«t?$âZX_?&
<oLÑ?$-è1¡[?ïˀV/?vÍ'óßjD?hWù†8­?dIíþVwÓ?l'°†
¿£?qC¼"ÏK?ï×÷xG?yfÂåiè?y'OL\7®?u†Ä#ʇ?'´ÿe?fNµøyhÂ?ï©B¢¼Ù?vє;oš}?{.²LIÙ?mŽ /ͅ?pH^øå­º?j*"ÊCQAGN3FGL J0618.2-2429@lü1 žÛùÀ1Ï~¶ß%À:›¹.ŠWÀ;ÆĹØÔB?é4Ê]9tž@Ì9¶3k@U'1>¿ß¹Xôk—¿çöçMµ6¿ägÄäÝ¿ïÿ´ó‰œnAGNbcu?îŽgÖlÍx?«I

¸?ŒY',¢qñ?"»ê—ݯ? 8ОA?¤õû¤—•?Ȝt™ž»Ü?Àͅº·˜?â&/Ø=vâ?ăÎggÔa?ÎÊÌkhž?ÁYBÄÿ+¢?ê™"ø0d?¦ç â­òˆ?·X:]+Ñ«?Ÿ‡2JUŸ?·Êøû«4?ŸÔŝ69Ö?Ù;àǼ¨Î?¶hf=±c?Ú·ÁŹÍ?ºwK·Ÿ¥3?ȼLÕyL?¯™µ9Q=?ï\‡QºÕ ? ¼' ôOõ?x²™ö+Úë?…EìÞ?Œ"Þ'B'?›`\p $n?܎Ï4ÊѺ?Ç&£‡?ؒVØšW?Ã&é—øt?Ž³æ]'ß?¹،þ¾}?í:kOž?œçýöR'¤?«sw«d§?"o¶:?¤Œ4ªwO|?'iÃNZU?åNM³ð?­bcû¼Ÿ9?Ðþ•»ØL¢?¬9žØÙܑ?±";p¬V?•¤À¸C2MIXED3FGL J0618.9-1138@ky /µÐÀ(Ø´¡\ÜzÀ9•o"'ßÀ;LžáØÀ¤ê…š^@	Ýr"rl@ÁƒÿÔa¿ç8¨¢˜h9¿åjŽ‡[˜¿çMû¹§ß‹¿ç2uâ@ AGNbcu?ï!'D¤…í?™Ê6¯ë?…–r­?"ëYÆ>?'KlXüm?•\—6–T?îYù^XÙi?µ®{Mr1r?Œª±@•¡†?¥YTms)?£5½È•3?­ñBã·Ä?ëBPÓ4Îq?§ç–ƒß?©¬ÚٞÐ?•ð£úB<@?¹ùŠ$o?¡ÙYwñ?ëÇ,h­'?¹#ÀCÒgÁ?i–¦M›º?yéråò­ó?ȵyQ®?¹$`	?ï|ô•Ç/²?'\"F×È?|rÔOw]l?†6·Yðw§?'‰p\Ù|¸?"pãµwÈ?ï~1d¸!«?švð‡Bþ?qËrT:OÁ?…¬ë)0h?‡íž;…`?'7‹¡M0ú?î]ý÷'N?"Ýå¯äã?–¯ñcf?‡cABëb?'(#8(
?Š‰ö"*ü?îbÙdÆå=?¡"»Hz?/Oym‡Ëo?E6=í¶þ5?©³7þbá?¡z\ªŠ_AGN3FGL J0620.4+2644@g6§?tŠ@‡'ŸÐ€À:F…íë*†À;ƒÜÌõ¹?Òi)ðûfy@µfEjC?úfz€NÄß¿ïÿüØ`?ïÿ›ß*ž¿×b÷ÌT×É¿àîúz¿	AGNbcu?ïÝq"W?m:è®?O‹K¢áÔ+?QÇH
/r?k»Ü¿ÿú?hŒ†"h­Ý?è«õQí;?ÊJ&MáN(?±ñôw×??³ ­®"?§?ÄÀ2þ—¶?Ğr§|T?í"=÷ðp?œÕûâžw"?"ùøRL?'2ˆ¼¶?¬¿¢ &ã?™K¯6Dq?é_³»#à?·'æɉä?À²5p`v?³!Iet"ÿ?³ž_¼ì–?­}"صD?ïï/cMŠÖ?Zuë'~S?<u"Ðð?:IäªVÆ?ZƒøÊ¢†?WP\õÀ?íèÏÉù«?·än] ""?"aWó¿é? ÅÚg?§ÂW GU!?°¾Ê1?îë_QŸ/?bñ–ú§?……@a¾Ë?y"ˆª~YO?—Ñu—Ë}?Š	H¯ðhË?í´¡w*ü$?œÚ±Š(?¦	U-¨?•ç.«l³?Y'¯T,?'>Ù$aÏAGN3FGL J0621.0+2514@gcRàãG@;îN.ŒÀ9:ÛWªÀ;:‹#µî?ôø / V¢@6|CG}m@],¿ü"Ë?﵂·ï‰Õ¿ãèðjwµ¿Ý4À£ý¿îÜy'Š~PSRPSR?¼çí‹D}o?·Ø$Ñ°?ã¿á×ËÙ?ÉRĆ_ޕ?Ҏ"ÙHò?ŵyt
>?¢¯Ã˞?©ùJ¢C>ø?âªËZ(aë?ÉR(ÊW/D?ØjSSlÂ)?ÉÙ.&{?Ðʉ·µu?²>ö;lMí?⎇‹`W?·p†bË T?ŨLÁ4úD?©ÁÀŦ"‰?ǕÁÜŒ¯?±äq¼jZæ?áLL¡Õd?ÂP§€j§?ѝw£®#?¼šÊŠìò?ÍöÀ§œß?Â%t—	O?âã¶Bò˜ä?Ç NEŸ?Æ{	1h>?½J‡)ªs?±€Ñ»bÛÜ?³ÇŽó+
þ?ä%—ê?ÄÝ3¥w?Óx±E÷tÛ?ÂßHv?à&˜©üá?²óLDO…ç?؜í`u?²¢»Ô/H?¼[u¾ëZ#?¡ÌÛøO6¾?Õ%_íȽ@?°½'Ÿ?àk	¡Æ?µ¸Qâ€%E?ÄðOþg?ªXž'&ޑMIXED3FGL J0622.2+3747@eüãŠ	@%éW€•ÓÀ8¦'¿aª?À;…h9¥=<@4ڇöY
@èBæ.¢@Õ.=Ú¿Ó¤ÒrS.¦¿åcR§0ŸÊ¿îg
ɐ4õ¿ïþàf˜Ì{PSRPSR?»9‰A:eŠ?Â1{xp?ê½G£#?Å8O‰¢x?­¸}$6ù¹?³ðíª4õ?oU'îÓ?}ñb>÷ª!?í{µØêg?·†W9c(7?¶ûzN–Ž?·y^è?Ìæõ/'Ç?¯–à;Ey§?ã¤Ýåmâ?´a/ce˜?ąêtA_5?«ù¶ÂwÈß?Ž©;UÊ"?"HófM°?îªYF‡Æ?œ‰Wy…õD?›`9€É í?—áU&j/?¼$	Ó#%?½žÓráÒv?ëpáõ±{?Á`ˆ~ǹÆ? ©Í'@X?«Ñ˜*&?aÐÝ@€?Œú%i~ÆE?ìó'ûaN"?´óå˜äB?¶7® /—?´-,Ûٙµ?Í­TšèÏ?±I2Yk?ã֘R?š?³è	åÃ$?ÂøJ¬È?­•''ÒÔ?ªïij'?"˜ž SAý?í°´Vš|ª?šcRÿo?•É–\Ydy?Ž?¯ôÈËPSR3FGL J0622.4-2606@m:†
¢À11 ‹ü"À9u™	PâÀ;Q­nb´*¿Ý3šfž±@ T^Q?ÿÁÀTCy¿ã-¥+ëb±¿àøÐ_Ã"ï¿äª!|&—¿"/YðóXäAGNbll?ïúw~Ló4?:ÄE[\i?;?,?yšÞâ§?Cp'*Ìè?8ãJ`drÍ?†Zo?^iB!?lÛNÞq?}Û{¸Éd×?"Ùœ"~¬
?"L÷ö¸Uâ?ïïøä‹?‡«ú%gÆø?'Ë"ôé?s¸¤TFS?'üCõݙ!?…¤'Φ?ïG°²;?'•5k?R¾j;¹'?&"•@Í7!?‹÷n‹ùÈÙ?'Ë;œs?ïý ä³ë¢?#Ï%þ¨x@?
¶ÿpÜÒ?p(ìKŸ?.ƒõÆ4 ?!²-I:…?ïÐʚÛ!?që
Ì9³?Wœ$Ԟ»?Uîe:¤¼?q³©Ê›"?l‹Ò
°^?ïœH¿¦7|?wO×9}q:?seaÍ0:'?fBUâv‹?~v>M&$0?s¬0Gâ•?ïêpY.o?Y®wkl>ý_ ¬!Ñâ>øC÷±Í+?eTè}km?Yý3ùªòAGN3FGL J0622.9+3326@f~¿p@"P(ßó>À7_ÿ»6¢SÀ:¾t_Mm?ñmóþ¿ä@ $¥Z—ü@¿"|üÕÔ¿ßô,.©ƒ¿äʳ¿âÑ£˜˜_¿äŘQ´ÂYAGNBCU?ïée¦ÅH–?d	‡ßy?:
/)-?6öÈcìßæ?cJ7ߧßD?bÏ«G˜¥;?ïT¿
W?¢Ì#‰¼?pü–8C?'˜T×k?'`ߓÎÔd? ÛÒB:^·?î!¦ß¹t¼?œcOm/ì?')â€çg?‰@;Mj?¤Ñ"(@…?—a¸@s™?ïûµÆ©zÁ?RV
ÃÙÿP>Ó¢‡	Y1?ÅÛeaŸ;?AŸ\
1k?RQ&Š­Â?ïøI4?L@Á¶(f?-<e½ÈB¼?(¤"‹½?GŠ©†]'?Hw×ÌtÑ?ïÍNÔh;m?€âF9ªÜ?Wê•ÓS?Y)ò§Ü?s•›îé
?|1ƒ(ëð?ï)	mßMû?ôsÇÖv?"ٖžbb?|…ò&ßL?Úå}îyb?†Ò*[}'?ïÿeçC#I?"a‡ƒ_>º"qÛø >Ò!zje?ØÎüŒ?G?"YÔ8pgAGN3FGL J0623.3+3043@f͚€If{@ ý_çœ1À:,üۈQsÀ;«Ú
þ?ç#½É_ì@[ۓ9-H?þJ/ßÏ ¿ïÿö¡BÁ'?ïþ¨©Ú¼?Á¡í—÷'¿æ÷ãÃ÷€AGNbcu?ï³[Æáb?šc¢Ã(µ?Zñq$¯?b="è4qI?´nÁ…š)?™ö}T§g²?ä'öbzüÿ?уoîqڅ?Å^ŽUì?ÅÞ&Ý©-?ÈìÇç¾HX?ƶä5Ò¨b?íð?;»S9?œiî"‹Yá?'Fy(c`?"Æ'ýÇa@?§Øϯ=5d?˜ѵ}??ìFe&Ò?»i·¥Y|"?´Äç#ó̬?¹ïٟ̗%?¢àÓr…?£¡3•#€G?ïÒx¾ØÈ?–Råߥö?A÷	Ð<u?Ho9ÛìÖ?tŸÂ"-ã!?–8ZV¼	?èðt³Aq¡?ËÇ+©=Ò?½i¹ 'ÛÅ?ÀùUîìSÈ?» Å̗7?½"ó9¤*?ï×ïÚ]?ÁeÇ!?'çx郎V?yµ×"&o?•+¨'jW5?‹½"UŒ:?î%Ø\"Ó?¥<K‡SK ?¨Ml«‹à?£%/ª°@?…T6WÓ¹?'û'ûAGN3FGL J0625.2+4440@e8OïI@,ÈFŸ ÂÀ9`+½,aÀ;'½ÝEÀÔ?–HDƒw@ºûø´\>@^È b¿älAÒæÊØ¿ãŠaçÚ"¿ÕÑéÝ­è¿Ý°6ÃOd[AGNbll?ïî6(}o?ZÃÀX#e?>0̎¢1ž?3«g*áj3?\|1½?Xì«)±¤?ï2e¿'>Æ?ÝÿDÜ7€?zÊwêë™?v1îCýÌB?".o±qZ?š'‰2£~:?ï
ûȈ?†Oþ
«X?…½Ìs!?ye
ì!6Á?'¹?–x?~(ÃB¤†?*‡Ï?'À?"'×?hc/q÷°?f՜øq\ä?£(4Þ?'Äb|O?ïøQ¯íek?eLN"!?2I–(ñ?$æ§gÒÄ?E±šßèr8?e+p8Ò¥n?ï¸âÐÍÁ?'I&§ñ‰?dß¹xèE?]dìw\å?yŒ²½#k?€¿Œ'ª?ï"ÅFƍî?sUN¸‹&ƒ?x¯ "!…?mÙª³IÒ]?|î<	KÓE?bÖÛzÙÊÀ?ﱕ•Â¹<?oe["2z?[Ã×[Í*s?IÕsd#´œ?€"£€™?lñ¿RjJìAGN3FGL J0626.0-5436@pu¨€QÉ÷À9ac€X€À9§Ú¥ÓdÀ;Áw=N?(?ÑÇÓÔ(
á@ã&?YÝ@]Ϡ׿ꬽo%–¿èñ2Á¸
¿åqh_åÿ¿ïþýR•gõAGNfsrq?ïòkwÕ?Y­Ðè I{?F('\×n¬?S• )šqõ?Pþõ*v?JfáxÀ\?í0²µtk?±·ØŒp&´?Ä"²¦i?›\JEØÙ?®͕¨&?¬ÈíXÙA?î£w@Í?lTIÕÍW?—Ò¸³¶?…CsÀH§?"¾_F˜‡ú?ƒÇE(?슰¤‹?¨Âxæê±ï?¤Xu?J?"¼üÉ_r?±ƒÀC›n?£úF‡â?ïöGõip?I'±W´'?Ag…5@?A0Ó«7úŒ?EFtp]?:SALÑÁà?ïM©ÅÐs?•}íS›¨?†""×ó+?€¥H¬©ˆ?'"9_&"?N¡0ŽSš?ï<ɂâÀ?€È6S8ã'?Žý9½k?zängY[?'ãø™vŒŽ?oü3…Ôò?ï1V0°™]?†'ÂØÍë?‡÷»Xž6=?rø՛:?‹²¸wË֒?'ÃNÒ«ûAGN3FGL J0626.6-4259@obY@x–À6hŸä6vÀ:!¾ê‹úuÀ;¥ðÍ]…?ôÁwAU
@¤f&O ?ûÖÁM½£¿æï"VZïT¿ÕËèÒ£ĿƝ_d‹è¿Óś¿}r¶AGNbcu?ïzŸ"{`…?'‡´âØV?ƒb…6-_?ˆMðº+y?{ë3UEt?¤Òcì?ïí¢ìdÔ?z)¼½?}èUâ¬?†á\ý?•(6[ÚçÛ?—2ùÛtÎ?èâÒ8­¬²?±ã™%À?¾"W†¤Ÿ?©ƒ'å(ü?ºe_ãõÏ?§¦ýsBI?îÅD?¤îl<À\?‰xD±'×?–­c¾U?©eë¥é? >íTñbÈ?}‰º÷?Œ}žP‹?~Uÿ-¢›?ƒ"ØîÙf?qÕB)(?xÀxä–å¯?ﱒs¬íV?ƒÖA•Iœb?eȤÙo›º?b]Ö¨v_?|Rsº×>?€î+Ç¥	Ö?ì[<Á¯ì?¦›|°?²ZWmé˜? ´\V '?¥šM\tã?–APÌ.ù?ï.·_Að?¦Æ2;Ø?š×på|c?ˆmg¡?†·P´"sÆ?ƒ&
@vÃÑAGN3FGL J0627.0-3529@nnƒ¡	ÐcÀ3øÄ!HÀ8ÎFªß<;À;*½•!dÕ¿ÐÓT;ý˜X@=B´Z?ýåS ¹^¿ç'chP¿ÓS0¹±<#¿ÞE]i‰þ¾¿Ø @…~bAGNrdg?ïá!—÷¥`?f¯³óö?OÇÙ茫
?Fxў}äô?fìqƒÅ?d‡ÅP—ˆ?ï8Ù~%&?œŒNðb…?uùâê¦h"?wã
?¹?"fWwá
!?™¥H¢¶B?îcOÊ\sã?"°ÍEv4m?"E3Lîu?‡‹«ºñh?ŸPÓhX•)?ŒëxÎ6É?íAÒi*!M?›|K>½Œ?eÚú—ø8?a#?iß,?µB"âì?DbÅì?ï°÷©;Åu?µÉ¯¯š1Ñ?'§¼U†ô?µÎ âë?K¶ÞêC2"?Aæ†yÜ°à?︞»—p?ƒŠÿ¦?a	=ÏÄýä?^5Mõ@[?{z'±bÌö?€í‰Q>3\?ïSóìµ?"Jˆr~?"hÉ\õ¸J?|QøCJý?†š;›…®µ?uVwIg,?ï)ž×Ø*?z}&0À6?SŒxŸÕ&?CÉËå°ô?™—D—ÄV?yÌAGN3FGL J0627.9-1517@lãø¶À(hß½jYÀ9óEî ÚkÀ;p©Ã³H—?ãÎöZS#@µú´¼Šµ@É£àDxÖ¿ãhD"œ™¿ï;Ât•dg¿Ù‡Èö?ÙÜç&•@AGNbcu?ïï¬Uˆó"?`7+MQ:²?.4
â¼,?0m†
Y–è?\àÓåNߛ?^Â}Æ°Ð+?ïDzޘ|8?Ÿ«ÇO§‹‰?xƒ 'Ž?‰
Þé?'O¼Œôù?–fs@XN?íi¾ô᭞?ŸCïÛÿ÷p?ŒNã4d­÷?vÔÿ~óu?±(+ñø	Ï?ž
%\@·?ï¦)
Ú"?›§U®ƒ¾?Fcìepù²?en*—¬}?œ˜y´ö?›¹µÄµŒ?ïèšÙ¬ü?q¢fËÐ?)Έ­Ux;?1<›ƒd™±?fP|Å"‰m?q@9d#bÕ?ïÃ$/½»k?:*®_eu?_¥fNe?bÈ)"°î?v"Žr¥Ì?z¬:{¾÷©?î.›	—i¥? ¨üP,š?wŠNfÚ?bòÊx¹Ä?ª%–>†©? ºƒ˜'3?ïޞ.[?q¬BòЍé?6Åk3§[?K®ªºEH·?n‰@Nݽ?qÙЗºÎAGN3FGL J0629.0-6248@q{`(^ÄÀ:oc€X€À9ʉŒ\`À;ÏXK±?Íã¶ÑÁ\@ć®à~@Õ$@Q(ç¿ä}©kD,¿ãA'á2y¿âЅÛe…°¿ÔsºH!AGNbll?ïÌû҅Ç?sVÁ þK£?N£¼,¨G?L–£Uê0?u©Â#®s?q®•Ô ?ï'¦ÊڄE?œB†´ÐÜÆ?wº**òW?w†le`ÜT?•x"绯?™Lýص·?î"r,Üò?ãlÀUl¯?ŒÉè"?z£~–|7m?ž«²&×{?ˆÚî9SC?îk·µÁr?—C›4?t'VAi?vIßߏn?¦´DA'¿(?•øWZ¨ï­?ïðsq«'¿?_0ÀŸ'`ü?8ꠌmÝ6?>J$B‡K?XÞt[Câ÷?ZdTÈ?-—?ïµf}É%?'¯ØiEæ?aµ½ÒŒ	?bl7SÎf?|q⁦?~ËMTGY?ïƒ076?qÁ/Ùa-¶?y -?e#»ëVçJ?'¸óq¿D€?gç¦GX?ï³ÌI*|'?r:"y¹ŒÏ?]õèÀlmò?R×,QÂø?~œa!ékâ?pƒ8dæAGN3FGL J0629.4-1959@l"†_•'ÍÀ+Mûþé‹À7ý0T[¡çÀ;A0Kø&?íªJ
aµ@NkåuF@u'A8¿à
øe¤A
¿äuŠFHx¿àˆM-Ê¿ä"'J¿ä)AGNbll?ïöàzºÂo?L!*nœ?*FšÁ?&¼¥òGLœ?M÷"qØÛ?Iô=?ïj•—xÏl?4–mfÌ?qµ,B&Â?rÐbeFG	?Œ€ñQ;‡?Š·~ê"G ?î¯Xãpþ?'!çqÃۚ?ŽI.r.F?€Æ8þã.?›M¾ÿΏ—?ŒÒÓö²?ï{Ûßþò~?‰6œº¯jœ?Fސâ[ÝÃ?R>1UmÞÀ?›éu-?ˆ¶"ׂÂÄ?ïüR-kÀe?2ã¦þùµ?!Ĩ»³?"("ÿH¿?4æ´VÊt?.úÞI&
p?ïÎÆÏ)?â?ur?þ<ÅO?ZáqÅK@t?Zæތ`øž?qä<Ú2á?p½Û²^²¡?ï^mU¤?ƒê홪òA?€qÔBÜÝ?w§C½¥U¥?‡òê'W†?~mrW?ïᏛ¹@?e!'õ´@E?:L:ãB?1Ñ?ë!»?k'gðk?d‡ŸÄõs¥AGN3FGL J0630.3+6906@b6`RP/@7b°ÿèÀ:ŒçìãÉÀ;úÌh"ÿ	¿ôßa.Ä
¶@
ÈÖ\˜‡@$ÇÛØX¿ã°»Ë·gпá´å]ÍÞ¿åR=‹7u¿êf:3Øt¡AGNbcu?îáD]Òîû?œeïP¸Ýµ?žõ(ta?›¦‹ÿÙèµ?s‰0›Ia9?p#…$uT?îâÌØáŒ?¦C`Ê<œ
?'gÈ:ð+?˜ÄܲUÐ?'?dƒˆW?q"'›?ìË=8ÌÛ?ŸŒ\Ǭ'?ª™8ܓ?–+²¨Œ»5?¨³'B
ÒÇ?'ÇL™Ük™?î•H&4r?Î–sȚ?ð':™"k?¬ÅÁ äU?§¡®m?˜JƒSS‡?ï¡Œ‡Ò?"kžC€h?ƒ†ØфÃÒ?'ÁpiqÎ?`Ë`6;?[FªÝ"m?﹝ZÄG?‡¬QPVd?oé›ÃÍ8?r?ÜÑâV?s~ㄥ
è?€aV¸B¯?îŒò}q«û?'G5n'ÜÂ?™ˆ:‰|?‰@L×?"ÙvJ×a?'ll«ø~?ï«ðWQ±µ?vèýÉ[¶…?YAyàRMó?Vœ~ÏOº?Ûºô°³?tøÔ¼× AGN3FGL J0630.9-2406@mí_‹ÎÀ-úðþÛ<ÒÀ7ßEó)WèÀ:°3cÛW?èÚ^t™I@—v2â*'?üó'_?€ž¿ËQú"Úgë¿Þ~OñQ^¿×¾!K²¹"¿ÓNÙ|ˆ'´AGNbll?ï¹{g2å?|´XÈ}6©?hâÎËwõ?qü—…Æ?vÐäáÏéç?ræÉÒ?îe$¹ë/?´ëÂU³7?ˆÈç
`}Ô?™kô!n?£{zö ?²ï͔>?éd49æ	?´Â9·6?§°é%ú¹»?šžK ‹}?ĂôÑù‡k?±öUOU?å8¶ù.ˆ1?´Û»áGL?‹7ßx²˜?ˆˆw_p[?Ô´ÓÙmç?´á·…0ä¡?ïÝ4h^Ûz?qœ {]]ò?Y:Jù«V ?]c^k'˜?f.qçÕºþ?kÿCž®?ïB]ÓÎk?¥žÊaá½?{o­'7á?†Ÿ Jð?ØqÔUB­? 1¨"Žeÿ?ë¨+ºVœ?ª;Gò·ÿ?¤ƒê&l(Ý?šu·µA?¸|­µ*/?¥Í=:<¼?êãµE‹iD?£‰Ò#¿Eý?2vÕ1f?yÔ:õM?ž	Ñ÷Z?£TéÊ2ŸAGN3FGL J0631.2+2019@hêßqêÿ@x€0¥À9fۙjZÀ;˜K»À5¿ä«—Y3´@st:9Œ¿@®èŸf7B¿åšqҚ¿éº€6œY¿á¿3]¿<°¿á¯hþ·_AGNbcu?½¦ÐJ?«<×Pþ-?LçJðì?H¼ù*|
?¤r†ûÊJÃ?«0ÜÉrŽä?í G%X?¸è˯6&?'ô'‰¾ý?"1¢ï––Ô?°Ÿ4…"&6?·?þk×õ?ì=ì6õ_"?¥×žÀ}'¯? 5šb3ª;?'
$Ì1)??µõÑ;.J?¡ôM¶?í-ôVËá? xL_¹?PPÒ»z?L=¤ƒ
ã	?¶O×Rìõ? NH¹Sà?ﲡ¿û$›?Ê€.så?<Þ¸53-?9•Ã­
yv?'pš7hÍ?¬àÎUpÇ?ï`'ZÒxL?›¿¶[=µ»?e®4;´÷š?eϜ
Hc?'9î'M†?™üî`lè'?îÙ|)'8?'`·OâìI?Š"¿öå
?´›Z•?—¿â£[Œ?ŠŸª»ç?ï&E-Óð$?fË°©ëË?AcÆþv=?0êôð.ñ«?š¬=ݜ'÷?5àrØøAGN3FGL J0631.5+1036@i's`Iì³?Ýær¿~õBÀ7ö†
˚žÀ:ÙҢϣA@– ´Ö`õ@
ý6E'@?õ8{Çw¿ÕF
ë_¿Ý.×výk¿âžržzv`¿ìO^\#8âPSRPSR?TîË	ÌË?SBtÖØõ"?îø'Ó#J?žK0~B¾%?Ÿž¸è>mN?ÂyŒ³Ø	?Cº~5ž?\ôÊls9i?ç'""?ºÿZNç*?ÐÕԙ†	«?¹êdÒ' ?¡w•Å›øf?–³šß…ZI?ëÝï""©?¨Mš)Ç?¸T¸"!…?£'e®ì£?•c×£'O?‡X²<¶fD?ëP"AÀ{?ª=—&ø'?Àt–Êk?§‹ß-Ü?Lðã•yç'?U7Ûʧ¿³?ïFVSÒB¶?"@™·Çc?–M®b>¨?"¹<î¾ÿ?\×Bž˜L?n ¦à	?èÉ
ò'`?²òƒ÷·U?Ì¢%±aÙ±?²ÏyIså¡?±Æý¨Rh.?¡ˆ"nEJ:?ë8¿±<E?©cþ'œÉE?´s
(ÙÛ,? ©"âe?¢`»Ù>Ýý?ˆ;_+Ó{?얐Ù4B?í
ö<ü˜?¶:팖îó?–çp´jwºPSR3FGL J0631.6+0644@i•¥¿­)™¿ôàÖ¿"ÕåÀ8"^ëGâÀ:–½öp4F?ù‡ÉûŒ'ì@ø'÷ŽÂ?÷­TF©1½¿—Õž'ŒŒÁ¿âà"~¿á7ɀ2W¿ìŒ˜_ö"OTHERspp?UKà(7l?T%è÷—¨?æáÒþó™?Í
"»ÍåÀ?Ò'ñ¤6o?Í
_RS''?l¹°þI£`?€Ø¿:&
?à2hU‡y?Â4ŸÂ±¢?ßa»ò4|?Â<kåp!?¯ Þk"€?›n]{'9×?ä~ü½§7?³°aH°£?Óë/ZØá?²ÕSz*²i?°û'þŒòÉ?ŸÚjýÌ_o?Ú;÷<Œù"?½"醖Ý}?à'°ëV?¿`z!Èì?kQ6<sÁø?¸
×:Û9?è;X|Á?ˎ۩Î3ï?Î¥Y5¦U?Ë‹2p$?'Ý_Wƒ"?•Ï}±O¦ƒ?áf–T>?½>êÈžR?ܛè]êH?¾àEÐnÃ?Æ/Kmÿž?¬r3Æ?âÓÎÔí`I?²¦"_x)•?΁y§¶½Â?°t¾›"?¶QæÝD>H?¡Szy¹l'?á9õfÁM?²Ó0X×?i?×ùT^jÞ4?´áýÔEˆMIXED3FGL J0633.7+0632@i£¿YFÿí»8 
•
À6ιƒCì¿À:Z֒Hl€@Ï)à#@Í@Vð9Žl@Ãë&Õù¿ÒSŽ:žj¿á0<<‹'¿æ9vTH¿í~Žè ÷PSRPSR?51¾w£?6F8t…8T?ïÓn¢¨"'?x~>™Í¬Ö?tõ'Ã+ƒO?w½IŒd÷? ûf!vå?D¯{BÊ<p?ê"eÝKía?´Ýƒ¤öÖ?Ū)²‰ˆ2?´Ö¬?†<ªWh?ƒ"ÂñVlè?ìÕ¥aà?¢1^f¥–÷?¶Ží\'Ý? ‹+Z¶TÇ?d#'?ýW?^/µ²¤a…?í‹ZÞë)Ò? ò‰ñ¹t?³öè½	? |#ói'?*}¼ ©?0pSÕN?ïÙÒá'¼v?s›àBÜÈ?rB¡u¾¢?sdoߍü?:uÜ֞j®?`ÖIð²
?êbÅøGNô?±ÂY¼•å3?Æg­1ë¤B?±ºu×#'?'ô²Ï!+?'4ǶL'­?ìîÈaG"?£èñIó'Þ?³ÌmÊ(›?¡zNW‹Ø?lKÃ1ö¤?^Ì<aÉG?íêKúÄ»?•+[4`ã?¯–édb?"IêÚ©Ú/PSR3FGL J0633.9+1746@hdA¿½ð'@'H$\À3L­áO:ÑÀ9=XJ@Äòýãñ@¶¥¹7™Ÿ?ôP'Ldë¿ÀŠ(æ¿ÚeR˜[߂¿ååðy+¿îA÷~§$òPSRPSR?õÜɜ7F?tÂa<'Ç?ï<ÂJŠ4?²¡ðÆ :?%qÙ«_?²~c¥oO?Cú–9+ø?{lÎdCw×?ì­Ê'Þ'?À¿9€w?ºi¹à"ˆk?À¦*käT©?pëÏ»¤dY?uÙÛ<túý?êmV¾Ž×°?¯FÖh¬çª?ÅÃFˆœé}?¯@»½ø÷ã>Å襡€à>íðLÝɝ?ï³´IÀŠÂ?Š>`ûÒЛ?ƒŽôS<Q?Š<lÒB*è>ê5þ…¸Šw>ø åR»«?ïE¹95ðl?°''×™Á?—E'Ñ
Ø?°«¨>Ù?[GঊÏ?Y­•á?í¾ieQò?µÒ+œSÚ?·|í13c6?µR²x!t¦?wQ7ƒŽ2?'˜:\Vè?êOŠH[?¯QpyÔq?Æ	$UZ"?®†¹y%3U>ºÑ쏶2É>É3У²¸?ï™"gwÍ0?ƒ  B}ñx?‰¶‹³-é?ƒÅÁ`uPSR3FGL J0634.7-2334@mû 1ίÀ+ýüߺ[À9£€)†À;ëˆy¶¥?欠tª û@?s­KÓ@JE Eš¿¿çm!W­TÑ¿åò¢ô@ã¿ëäTc ÿïÿL]?ýAGNfsrq?ïe¥—tí?"ÖT¾{ÙÉ?…ú4ÌÖ×?''3蝊?lBú\¸?kâÊÐ÷;z?æä-μ³q?È3Vú7¿	?Àh@Nhˆ?¶²}H˜?Ä:"¾É²?Áƒ­ê3ú?ì˜Ðž"~w?¡QəŽh?°JÃ$óÎp?™±!u›?¥ÝoÐP£?"÷ƒ?㶝¾õÒ2?³0)«75?Íò»Á.+?³‰±œª!%?Ä–Hg‰?«Ñ*`˜õn?ïÂÝ×zêq?xAiOo??vŸº2ÔÞ%?tL	ƒŠ?_Åh(Ú&?^ '?ìž4Z>~°?¸ÜªÓ'?¨â겛08?¦ƒÖ‹»?­9ϪXËÍ?°Ërð—é?îpW$e	?'h§­ZK
? 4é8yÄ?Œ"yÄÀx{?'‹Hsed?€.Œ-hû?ëj–êÆ:•? ×ݬUú?·V'Vƒ^?šÃ.ÌÜp?ª©/7ö?"@ë,´>AGN3FGL J0635.7-7517@qæG rѯÀ;)_JsÀ86
ÄÀ;•« éð?æÅ]‰ÀU@eºsY@®àI+m¿æ¶{v1ÏJ¿è]¦öh@u¿ë,͑Ôå[¿ïÿ.¶÷£eAGNfsrq?ïõ2M@a?UDlJéδ?HU£]<Ù?Oú'@¾¥Ë?Cžà÷Í?Cý9?ïUíî였?'þ­Zñ²?t¦ë!°®¦?tÎþ°ç?‡R›W?Žš}§ó?îŽ+d¨?È¾ªˆä?šéêL¶þ4?‰Üî½i?"P²™¤´?'%
éÀ(?›}'&?Š7(Í5?k|¹õfÂ?r#'ÅYÏÌ?…ÔyíÁ^ç?†áÂ'¤¬?ïúsÃú§??K Ë?:ÕLF?5H¥EH?2Rõê½´?0N¬;?ïÄÊøêÀ†?v©¦´ä"ˆ?`õÌ:¢³Š?[zŠè@¼?uY`§1?qÒæ½Éږ?ï"tgÂM?½,w«}à?Ëbû‰	?z=¨ÒӔ@?…Ì GR?r½b_êK?ïêBØ(ê?kò]ñ­ê?EÊv–B‡?BOX…j{é?`J ŽˆŸó?jt⎀ºéAGN3FGL J0638.6+7324@a¨ Àiçû@9¬OkxÀ9—}K…9À;ÝM×#gä¿Ñ{Ë6Žv?@.²§²Œ@笳¿æS<ã¹á¿éj;ÿE׿ä=š?\¿ïÿ©ü=RÇAGNfsrq?ïþìD¯?-Š#]›¥	?yHŒ]³?²GÅà%@?'2å[`Zu?*±~âà?ïwœØyt?ŒE¿ý±q'?{ã¸M9Ï?t†&h~'{?"&í°Â2?ˆH
¶t?îÿjWGö ?Œü[ñókÖ?Ñ!ÔwL?'ï/Wç?*3ÿ7¸f?…@&•â?ïtnl?‰tÑãÂE?pZ±t};?q•ˆZ/‹?Š"÷ٚ?…ï¨&̳Ò?ïÿý¸–Ï?Lìû!¢º?"0C ›Ì?Ґ]ڏ?6ƒ4?ÁάÓ'Q?ïÕ…÷Xð?p)ҙbåš?b¨€°s3¬?Yß!©ÕH?hCù;\¡?i+úœv=S?ïQOž¬[œ?'R<bÜÄ?ˆñH¾F‡?wð¼%j´³?'ºÏ£YŸx?y—â%£
?ïè–]é®õ?d´iL½?Eâlƒ Zb?@BS"~!?añfìÀ?càÎ՚4¢AGN3FGL J0640.0-1252@kæHÿ¸²dÀ ŸóI"À9æ´5&RÀ;UHf¡?à9¶{#@
ÔÍLN?ø3@¿bÖå?ïò>Çøþ¿àV³üyì3?Ëò«{ã¿ÌŸÀÿRõµAGNbcu?ì7ÚƒȢ?¾5fá'ß?h'xÖ§?g!å-Æ?½|–$U[?½Þh¢ù<?íÁR‡P/²?¹
>lý$?†Àó×|?ŒÍS'i͹?®gUÚÀ?¶ß©³U?í
ìªZ(?¢™"̳y?š.Ïx-?ŠtÀœ<â	?±æÍvbT? YoaP–µ?ìÌû¢¬µ?®ú¾¿Ç?j?c{ßÏÔÙ'?sLV­ÿ?¸üH…ªÏL?®âÆ_)&?î/,\Í?±¬¶:"áb?]$°Ž%»²?[Öû.ž÷?¬$vùp?±ûGIñ?ïIR(Ŧ?œ|iMš"K?qŽšÆk
?tÍ‹êø?'rM›ö?˜‹Û]ÙÉ?îPõ½ÿ ÿ?Í¼Tè6K?¾K:ø	Î?ˆ&«m?£MàQ?š8¯èoÓ?îý{µqÖ ?"QŒ¥BÚ?hⵜæ?e­›ÿ"jí?4FU:IF?'…zdtDAGN3FGL J0640.9+0752@i—]÷vÅ?ô}^?{kÀ9Ï!j´À:Í"4H?¸Vº£‰ÅW@
]lŽôz@rZ¿i6û¿äu§L
¿êÂ]B¡¿ê)^ž	¿ÑÒã|¼"OTHERspp?Ñð¨ãÓ=?É¢Oø³'?¨ъ¨Ž?©£	G?åûwNYîù?ËüžŸp{Ç?ÏäØvÍ?Ïlxž]Š?µz…ÞŒùß?º%º0µKô?åWy&?ÏðÙQ?µ?ãA³ë™/€?³e6f§ç?¿•½V*u?¦q^H'¡?ї(Òu¤?¯°°ôjz¼?ãÖIo­{?¿öçÃ.z?'º*BO¯?"+~FÑ?×7Ê|e9?¿ãÀ±>?âjŠÕ?Ïzí9²\?'œ6Üÿ؏?"
L¹3?ÙËg}ÎÉ
?Îê~ŒU–é?Úƒx"¯
?Ôï†&0|†?³³¯ gÊ?±é·¼åå?à'§ÎYò?ÓÑÙÀ¿è?ê®é‰"è?¨a*—w8B?°Pð,8:?šÃ"éŠ?º7Ç	Ç݂?¡q¹'É ç?ê¤Lºæå?¯.úÿ»¯?ƒ5ÓÏ0"?vّ©z«?Ä;oØ*#?®ÿmw<MIXED3FGL J0641.8-0319@jÙ¦ %9uÀ
gßbP­À9‡86¨2ºÀ;¯#nš?çÞKpåW@¬¡ÚZÔã@¢Êi²K¿æZ×ä⣿ã=*É(å¿ãÀãîZÙ¿ïÿôG÷ ÅAGNbcu?î¬"ËåyÊ?±šD!?€túÿÁ:û?¯Tåâ&ä?¡ "ú
?°S£àØ8	?ã~žÀí<ü?Ò&Õǝ8
?®'üÖÎ?¬µöAqV³?Õ0'ûX·?Ѝ[éñÜã?é®GW$?°€(]°ù÷?¶àÕl~d|?¢4 [#Ä?ÀxÜú[?0?«ªâEž´z?ëͽk8É?­RAÍGŒ?™ŠçOx£?"
ˆ…zFÑ?»/Zå?©‰D¢Ffl?îð†žÑM ?¸ú¼Ö&ì?rᖬ):?ì³Ò<ê?6Æu ¼¯?·E8'ÝV¢?ê'5ãoY?ɹ¹El¬ã? HŽ+Ê5?¢Psî‹Ð?Á¥Ûžn7
?Æ'«HKPê?ëPà‡­?©˜—toK?°—Of)1?œm³‡oÃ?¶žj­«›æ?¤B¬©¿ø?îNõ	¶?jqm=‹ ?'§©Xw?{³ˆÅlIj?¡¼Û9¸b¦?‹ª]GjAGN3FGL J0643.2+0859@i®ÀrKw@:ßkàÏÀ8dbzÀ:ÎÜq…~?ùûdg@Ú3më–@ÜN®¹¼O¿Þÿi;Ö¿ä»`ã¼õ·¿è|s±±¿ïÿ…"
ì'AGNfsrq?îo@ñ?¨‰ÅÄ£f*?cvãº?¢aj?•Ôw5?šõ¿&Ÿe±?çF…L€b?Ï"䕅&µ?¨ €ߞh?¨þhÄBBM?̽Êȳ?Ë}C¾ì?âAҝ=µe?¶A‰a?ÍVVMênž?°ÆÙ֑?É¢_=»Ï?°ÊT|5
?äÊc—î¸t?¾\9â#÷?¹~Ãh?Ç{?²ÛÃjxnÒ?Їõ¤©º?ºN1]½lÕ?ï+‡Ì×Ms? Ÿç×ä.È?'
ô±?•ütkøJ?ƒ
ðò.¥Â?"K
ý?ìjè`üð?À¬L{Ðþ,?;FÍÐË
? }å:Û1å?µYëF\9?ºÅÂ'k2?娐r"-?´*¢PXzC?ƍJàÛo?­0Ž£}e_?ÂÐu›/_?ªŒ¥¦~k?é!‡ÁÓO?®ýä<v?¸–'J	?¥4·J™&?¾t+å¥Ðx?¥\q-iAGN3FGL J0643.4-5358@pu3?ÈlìÀ6ÆfÙ×À:
Oa´À;Ç1Xg "¿òó—Œy§@Ùê†7"@Œy¦Žu¿êN=ÄAôþ¿×%ƒˆÇJ"¿ç½z_þ©z¿èñ04;AGNbcu?ïéÞ}Ï8¸?hdv¸L?`"½ô»%ø?f¯S6
?F3€–Ò÷?EXh¸r?ïbœ+ç†Ú?'K÷ã!?q1'P'"J?m`š…¸ø@?ŽÀ,dé·à?ÏÞÝÂÿŸ?î£r^Iêã?Žžž#1¬?–Q¡æͲƒ?Šø[Kîz?•@VÔ)?€'cZyØ?ï€Izâ
@?ƒ'úÜZ)†?W$n°s!?Yœô•-A3?	s&²?ƒG>Ú8¡®?ïôÆ÷~YÖ?TûÓPl¥€?OaÛhàj?R6Ué'?;‹üßÐ?7ŸH&Ïä?ïÎøI
4?rî¹n9±4?Y
OB?U
U=Ëæ?r>Ð?o³þ'yú?ïZƒÐjÍ:?‡Lpۅ-n?‡'Èš+K?'æ¸xC?ÍCV¢<@?tÖÂéªÄ?ïæg/ºï?c(œ;Ö¾?%sN?#z–©îæÜ?h?×)ÁU?bû,úffAGN3FGL J0644.3-6713@qX—ÿ›V2À9‰4ŸCý†À7ØýCŠÀ;åÉä?ìD™ùw@Ou¬ªm|@ÂÿýfH¿àý'²Ìq¿áæ
n £¿à½ëtœxá¿åS
æ&ÔÅAGNbcu?ïüc'ö?4ÐSËÂw?$ˆÙXÚ='?#¾3¶
Ñ?5@xì=×?-3î7¥©þ?øµÍœ?‹iSBלÞ?mßn±TÉu?}:(Vö}?…\æ*®ä¶?·þ¨ÚM?îñ	ûßèf?;®2×?‡pŠô¾—ü?~ÁCü_Â?–&{
C<?Šð®ºyIS?ïÐÂÝPº?w×8×|?% "
>M?@x°ˆž?võ>"ïÄA?vÆ։Ÿá?ïþzšûÄ?ðn;Ý?äeÈÄõ?ßøçE"š?$"Sëß?±%s³,B?ïÓ½ø|0±?qôGYj³?WιN$W!?T'®9øíè?p-Ud¿©ð?k^Noo¿?ï}œâ4¤3?³Éí³š÷?zkˆ–gb?sÓ¥
O?ƒŽ'°›ƒŸ?y±Ý^Eª·?ïöŠ³uõ?U.-Kzð<?ªnícÒP?ŽO£&AP?Q'!ùš™?TåoŠlJAGN3FGL J0644.6-2853@mÏ:ÿ°NèÀ,.z WŽ\À:_Ï2ÚÌÀ;Ä}‹F¿×{ٌ›%Ø@d‹šÓU}@㦿qð]¿ït¾§VVà?å	k©qRþ¿Üù»ŠA¸¿ëP"T'±AGNbcu?ï_¡N!~³?'¹…ס»?'aÏn`Ýp?¿JÍÜ?eP6›"èÒ?f^¤"c´?í–êÆ:•?²TÐ9Ya?™öÈÕ¹ˆâ? åx¥JM?©•ï4
 =?ª ­ùÍñ?ëäL Ñ?¨峒Wö?¶Rú³@Ýá?£·Æ|çâF?¥H‰Ù˜?"톿¥±?î]¸DT™?¢Ø=©Î?Ÿ
#:.ßm?ŸA¿éŽ?•CåÂm÷u?'JL^»<Ñ?ï¶È;÷·?€oC—Gòj?D+㼈?~Ÿð—u†¤?U^Øó· R?RÇ=)á?ï@x+Æéo?–S]Y©<ð?vBÇ×ù?|®n¤Ć?iܟ&?'fk>É[­?íЕýóË?›Û@§Ú×?©kîÂi<G?˜‰ ±ú$?"bÔÖ?†½&ýÊåz?ï¬2Þy{?z?%½#k{?t‰ùUàñ?r]‹*#í«?u\—«»Ù­?m‡èyù·AGN3FGL J0645.9-3914@o@ßXÀ‹À1À¶àÒ=OÀ:ª>,‹À;Á¦V]ÛÀõ‹¾åƒ}@Ê'D½t@'ù gÔ{¿êI»üke¿é
šO±™¿å«¤¶£¸¿ïÿ1¾¾íAGNfsrq?ïßiʞõ#?o•´H•¤?X¢˜¶Ó?]«ªÛÝ
?dE'B_Y+?gƒÅP8rÿ?ï;OM‰å`?™¶<VaOj?z5m:ºé?"D¤?%?'»ôq?"z§Ef­?í;=öWF?œrÈ®áӐ?¦méwßQã?'7TK?¥ÞDù— ½?'%Š™š?ï(\ãZØ¿?–ŒZۇ"x?LÚì¡3?XÊ¿ž<t?šD¼Á=?–AX(ÏÆÁ?ïí˜
óÖ?_Á nÑï?N¨S_(Ã?Qú£' 5;?UÆ%Æ:šÜ?Rêõîé1?ïÃ(Ò9Ñ»?î4§çb?_£^í]Õ`?lñ縲JØ?v'¿*\æ?zb}Iì?îœ7óP3
?Œnÿ¾Æâ™?šmÎ¥²?ƒÏó›_@Ô?'ý¿Qò¹?ö"ýRs?ïÛ`´~Tø?jÓ,Nè?@çW\Éì?1ñqߛö?r¢(/Ã?j¡Ç%óùoAGN3FGL J0646.4-5452@p†Z\FRÀ6˜À§¨À:±Œ7±G5À<w&0ì1?öaÖâOj÷@!VØÿ¶¿È]¢Pþ?ï¯ù͋äz¿ÚՕŽ7ï¿èÛ~re'ï¿ïþÞdFHAGNbcu?ÓNŸ©lå?՟ö˜«»Ž?âÝàyÕ.?Õæð¼HÏ?»Ø¸é@ ?ŏ&—!!ì?¹ÝV-šS9?ď¿¡Ò3z?æ¡]˜ó"?ÍñAҙ{£?ȍCrÏ?ÃÀ.¦(?ÍÆ "Ñâ?´åéޓdD?⵫<Ôê?¸²_?–óì?Çc3:ÊE?±»={ˆ!ý?ÚøF[6»?Ì_üŸg(?ߏ³´o?ÌE"<›$?¸§Åžˆ«?¼æÕw–:?Ê¥b8'?Ðh½×oÉ?ågnúÅ?Óâþæ-#­?¾J'³?ÊA^#÷«ô?ÎÖ"'‰ƒ?Ñ+÷Rød?ãxýª6ï?Ò½TÔî"X?ÃEç,–ÙB?¿JòÂÁ×?×
Qí]'?µ7¨i€?à˃ ±?´­ j¹ÊK?Á¤ô÷8[;?«â®À°$o?æÝÕ2ÌÜ?ÃѦE¤yò?ѺUç=;u?Á/EÔÖ?¡¿spU¡Ÿ?©,—­n(KMIXED3FGL J0647.0-5134@pOø!ïÀ5"Ð_ÿDÀ:C*È*§À;ڈ§ÙÎ=?Å$ÿÇSš@
âÖ¤fý@ƒâ?Ð¥t¿çÈÓ*^¿æb5a¶©J¿Ø–8¥³%¿ÑyFðKÏYAGNbcu?ﳅ³*0Í?†@ƒ™KAÒ?:TÅ«
*?:ãü>C?'Kìøô@'?…ø"ê¶o?îóLþ,ã…?«ÁE\ºòÙ?}éhùcº?ˆõŒiŸ?šü
«i?©Êü;p?î;#õõÝ?¤‰??'ÁÐt–Ä?|1Ë{?£młåÿÍ?ˆÅ¦ã$ÿ?îŽ)"ÄÜz?—CF'™˜…?gÜ ‹mŠ\?tþ½d–ÙÔ?¥Ÿ¯Fâº?–HÌÃ)ÅR?ï^‹ãÅÚ?·ú(mM–?`Ü8ˬb?…Ñ	Ç3n?'üfUe?µ©åæ"O?ï°(T.Î?…~ÛÓ%•?e,°pxÌ?p.6EÀã?}UîdC@Ý?~÷ØH;è?ïOËä?wÒh@Žf?€¸vւ?cì"ÉAn2?Œ
‡Á Œ?rö¸‹#Ã?ï³æÓDqZ?r
1pL ?[=‹œw~?Uð¿ôèœ?=3"Â=?p5õòîD AGN3FGL J0647.1-4415@o²Í ¯¢ðÀ3I`ÆuÀ:œç+ó¤À;ÙLhÏÍ?¼ýaÄYûc@]†ÎÇ8@Ás\f³¿ìôyI˃ª¿åÐhYíî?Æ ?ïìÒRzÌ$AGNbcu?ïc.N$®¿?‹öƒ[gûT?"멃\ñg?ƒræm¯öE?'HÂâIS	?~CLulpC?ëÎ7Ü÷M?ÀÎÜøHÒ?®Sí¥ÐØ¢?¸_
Zö4"?²dJF9-?°Ý¢1«4?êʇfwi?¨=ãJɚ?µ±¸ðÞ
H?¡mKm¹?³úÚø¶??›cyxÇ$?ìü•ëlӛ?²:%ÍÿX¹?ƒãŽe?™5#.uŒ´?´jï'K»™?°1tíæ²?ïCh&?… «"h½?yÈÖr»Òà?x.´{£¶'?~.ïrr?zc9Njó?îp`ÓT{W?©8mc=Ž—?–¥ÉV?š™£Ë©?›cы£aÄ?šÚ¿¡¡ñ?ìå)Æ*¤Í? "àC÷ü?¯AÉV©7¥?›4cË0´a?¢kšDƑ?Æ¯[µ£ß?ï.8Ès?ŽNÅk÷£O?… 1VlÑÃ?'$W/â%?^¢¡r?ƒ47TÖøAGN3FGL J0647.6-6058@píοìºÀ7ñàè@À9KTÛúg:À;­ÈŽyªç¿'t8w÷@ŸŠùB̃@±¡ y1ſޟÜaÈÐq¿åd'ït¿ä3Æ£_c¿ç,=¾&–ÃAGNbcu?ï÷#¼-ÿS?L¬óJ)(?1'è·Zó?5ÄÑ]ž?J݈ä
Q?F-ß(‹Õ?ï‡ÆLCê?qV,Ó	â?xGª¢w,?s¨žŸè?—Aq³?›¼¹,§•ë?ïàÔ§É?""|cï7?†Ù#$ûÀ‰?vRv¿ÙÛ?"''L
î­?}S]õ§€?UŠü?"v³8ò§â?sÔ|B=‹«?kqŠü«?¢+{ 5>K?"Éý9§®?ïüNAxè–?6¼eZ¹Û?"{2D5lÜ?#£z÷»ÿ?4PZ"‰#ç?/]؝ú$ô?ﴒÆþh?S£m'S©?c̶À†™h?\ŽÕ0±ì?{НA?Š?~ᤤRmÖ?Ë	8?mpü‰TZQ?tüM-±DU?eôáFÓë?|¿ÍköK¶?_žÊ@5';?ïº]
¿n?u/èîÈøe?VÛ´ÈЛ?D3Ù(Ñ?}'×µí?tv\câáAGN3FGL J0648.1+1606@hÅZÀ?ö@A.Àë­À:…Ç7bÀ;±'[¶¿ížðÆ|&@SöâŸòÏ?üdÞßHûG¿ë\Šfd§¹¿æ̶Êàl¿ØHZ¾"Ì¿ÝOŽéðÓAGNbcu?ïãÈi½R?e®?\Ñ'?9»þV»?=ád%ì´?i72®?doÏwHJ??íÇkø²¿ì?¹8ýr‡?ÓŒ¼áÒ(?ŒvšâR?¯]Fav-?·§Å˜…Zc?îð¾Þ;y?–ÍpüZ+?š{ü+³X?}:e	¤®s?§ºU¡¿ ?"Kœ™OÞ?îÀFQÿ?–mL M?C¢€_%Ûë?Dä'ûX?£­üŠX?–E‡:?ïów¯Aª"?[w°@ú?:¸Ï²þ.…?UZ_¹xX?Rbmܝƒ?M›ŽC
1?ïx•öÕg"?•ž¼Ü#^?f'`HV9?i®¿ZCN|?Œ5ú¼2ñ{?'Í¿'Vp?ï05¹«Í?…v;C™?1M|Ííq?qÔãÒ6ëè?'`¢!ëq¯?€òÃ]Ž?ïºsc¤ë?pÜïr|¾Ô?3P˜Ñú}?'`#ю¿n?€È¢BúïR?p ,º®÷)AGN3FGL J0648.1-3045@nÈ˒:À,BIÿ''ìÀ8áfãcèÀ;rÍ 1cO¿¼Ü+Ë­4@GÜ7£Û@te€¿æ#­5F¢–¿èZçï+á¿ãHþ®òf¿è»zóoAGNfsrq?ïüûv¶ô&?2¥œ—¡Eq?Ž×p f?‡_R°Ì?4Rmñ*;F?1€\.*L¤?ï…Xl~?ð»ÇõU5?m¸¸+¾É?~­Ža°A?‡;ÌbX_Ÿ?†œáٖ4?ï"RÏI™?†JÝ7ÂÓ¾?'Ê€©:?o¼Èb?Ê?–
5UOÒK?'Ö,ôâ	?ïî1û	Û?b—0.V4¬>þ}Ëso?{N=˓?a'
¸˜rà?b}'x}]*?ïþ¶™¯"?¢e?وØe?k{ç)BÁ?$`Ž|À?ÑRÐÆ;²?ïӄµE?sU3ìG7¶?W€€\(?UÓÌ
fÈD?p]òr¥nL?o
¦*ÛMª?ï'G‰ñÕ?sœË*rÞ²?sñB=‹RŽ?e¸õÕY¹/?u|hb=X?o
Aåb Û?ïüÿmðÅ?9"ð×l>éGhÐü_'>錌b)Áö?7:U›Zý?9oE@a5¶AGN3FGL J0648.8+1516@hߚŸ¾vÉ@VÚ`SaÀ8ÄN¨¿¨À;ÚaàŨ¿èÞn3ÔÂ@­@͵€?ýKF(_?ÍF:™Pjô¿Ôl.[ ü¿¿×``¹Û¿Ù-Á¼î‹AGNbll?î"
¬V_³?±/dý/Á?†}·l¼Œ{?"Mwú¿?¨?ç]³²?°‹ý:›	ñ?ì	Ñ'Oz<?ê¶ö)p?˜2`ö?¢½¾Æ\—Ç?¹¤Þ†³á?¿¹}$C[?ë36§ö˜?¨0Ã÷ì)?§#5ûi·7?"ºóöNª?»¬ËKS¡¤?¤AFYF;z?èȉiÔ1?´‰æ?Ø?}Ë[1KËß?{'$ÿßè?Ë£<?´iÔL´>?ìÑÇP" "?Ít²q#P4?‡È¬à%ø–?¤Ãʁ¯GJ?¶x¯ÞaÏ?Ì8qWþf?º‹??¯­3WÚØ4?ƒÞñL(?')À1¢©'?Ÿ¸ú5z[?§ä(Izf[?íã ¥kMÆ?˜…3\ÙÝ?šd§À
k?Šgi×7ž?¤"¡ËÖÓm?')ær),
?íMê)L;?ž§'¤¹¥?b³CøG
ì?V?î{Ÿé?´û响Ô?ž‡œvU¸<AGN3FGL J0648.8-1740@lŒ`Ëò²À!9ÿÖ•À9aéÐé'ÿÀ;%HŽå?Éoà<+ø@¾ß"	v@(Mß[ð—¿è`.'ô¿ãÉç'/y¿éѼø»¿åº4!xSAGNfsrq?ïï%•÷ß±?^ì;k%¾Ý?A<Ï&Ò>Ð??èÙØpU?Yliño?[¯ö@s@?îžù-0˜W?©)‰S_Õ?~dz"¶À¥?…ž»ß˜0?¢7v·1ÿ?¥Œ'³Áûó?îoqí$¨x?'ò'"+±$?–Ð"ð|?‰ßù>3±!?›ñÐzÒ?…f8Ev?î畍<áT?'sSøˆd?YÁ4†y8?]+—HçŽ? ¸ƒÈœÈ?ó¬ŒÚ?ïø»öeÍd?E/Lۡʧ?4ËÙPï¡þ?2˜|+Ö7Ò?Bª9ìÚZ^?>I`Cj†ø?ïn`O ý?œ~%"OÚ?iöý˜æÑ?mé.IïÙ0?þ úõ?˜îÃ$~û¹?ï]Cÿx	–?t'YA?'íªÓ&ÒØ?wíím*Ó?…ÁU@uË?uô"r¡Ø?ï·piÄ?n\‹ŒĂ?F´Ip{Ü?4ƒž¤ùEà?€Ù«Œ§?mºá íîAGN3FGL J0649.6-3138@n06¿DNÀ,d:a$ÞÀ9¬þ›{ñéÀ;`œ
è ?ͯzVˆLë@¸±¤þ&·?û¨² yL¿ìýkÆLªþ?Þý*ÍŽØ¿Ãsýyy#é¿Û­fѬk¿AGNbcu?ïàh\Ø¡?fÿLÍ/À?FÛñ³õs?B(ätÃÜû?i÷¬:VK:?d²/;N¯?î˾M
ÓK?¥-£	+Ž(?'–þn6g¼?…¢ßå?<·$ö­¼?¢"ôIÁÕ?î«å–1?Œx†¿ñHâ?Wõ;T4£?{¢;·ž?š×b_Ã?" šî/?îºÔ
)?¢ZÓ¬­ ?ƒš4U•†?fŽSd0ú?ªýË.}q?¡À¤ÑO ?ïñœÀÉ	?\õÖê?9¾ç¥eK?<ÁÇg]‰?V…Ž:»öº?Y…bËX?ï¡ä^cã?‹9gæ3Ê?gTXµ4h?bvF²̉?±Ò-³d??ˆA'	%ºò?ïp,WË?v­xY?~µ±IÐ?i÷`Ì*ï?"š_éÔØP?pÿ|Ó2h?ïLp±÷g?'*" a\ƒ?vö^4u?eÁVè?~?´cmYã?^ãÅÌ¥MAGN3FGL J0650.4-1636@lv²gÇÀÓþ_ìÏ¢À9.Wø™÷À;Æ폺ô?ðûc"xB\@håòŽ@uâÿi,>¿ÚéÒU'›¸¿æ[xt
¿é€îIõ˜¿ç¯£2ìÞ²AGNbcu?éöýU?Âјy)š?ÄÚÖx¥¶¼?Á™wWFÛ(?«¶·ÌÀ?§8©ø^~?äïïìXû'?ÐÒ¬¶½ýã?·£\ª¿ ƒ?´ ì?Ð7Hüž ½?Ë­åV›?éoOÝҝ?«´ó†,ÑÜ?·Ä" kÍ?¡#Vcò¯?¼/òaÿH?¢ï£GŠ†–?Þï£E-ËY?±)€j?È@kÞ~Ã?³§!N6?Ôð&ʀR‡?­»o
q0.?ìZapyò?À±á±"?·ý4Ú¹Z»?ÀWåçraê?"¾þ•ã$Õ?'j·~½è\?ëá>òÚ?ÅïŒõò5?ª¯_ZÌ`?°93OÔ!×?º‰F`óœ?¾Xn<YÞª?í/Ø>Qñ? Ï¥^?§f}i`Œ?•³~z·ß³?¥é¡µ™k?'y®J?æò"üH)S?¢qïìÃu?ÁƺNší­?Ÿë_¨êÂ?Âp¹ÀDm?—s‡1CAGN3FGL J0650.5+2055@hA}`éNä@"c.Àë­À9¶'Ã]À;Th®?C¿°[5ÑÎ2`@«–ÌŠ²¡?ø@W¿ê»b‹TKK¿ØêpY·ßÞ?›FAi#¿Âôû#ÞAGNbcu?ïÊ{ y —?tF¬éíw?RK:ž³ö?P6z'"µh?v/aóBø?rÈç'Kþ?îª(ÜÜÔ?©?û÷ë[?y¼Ð: {ê?|™5a›;?¢%Ø)<ÞY?§jà31Û?îbû°ÃŠa?"4…–?ê\6?€×µm9†?¡Õ¡­pX[?dÎX4–Ø?ï»,w"?"¾^ID>?3~†ê|¢s??'|±Çû?›Ñ®…zWÿ?"µ&ç:‰?ï퓱µU?^¡GÇïŠ=?<Ne,˜?5Áà`ôï?]ÅɖÌ?[ŸT0fIÀ?ï§ÅuY?Œ½È
z…æ?a}§÷.Ž?\Ò&9Ä?Ç³Ü}O?Š.ɲŠ-?ïLò'FŸT?…vH9º?ç¸'þƒø?y"÷QáÄ3?ŠÛ¦ä˜¶ê?±n~©E?ïŶȌ?n`2·ŽªY?8»®úµí?1úAÙn/ÿ?{ð9-/"?m²SI]'AGN3FGL J0650.7+2503@gȱ ‹ü"@&ðál—À8F-ù7ŽãÀ:мž_ç¿ÞÂrYzH@ 9#¸?ûˆ~žìiË¿Ób"ý[>¿ÜυÜé-¿Ð¦=Y°S"¿Ôà©3¦²AGNbll?ï×U«zÂ?n©ÄL‡*t?JÙl†j?G.8Ѿ«?pùüù—Þg?k«Y?£bR?îæšIur?¥è€HÄý¼?xwgŠ9¿"?x†ƒlzŠ?'Úr-Ã?¤4¼azh?íAt»­"w?£šUñÃ	&?'¢›î*?‡ð®/Q?±K³%¿~Ç? îå	0_¬?ìx·6ìü?£~–jÝeï?O2	å¡wç?MJ²©v?»ûâ4Ï%Ô?£l×ñMr•?ïî'þêp?YJ‡­?<?l':¶?6žñON1?[ì+øÔ*?Vþ"‹…§?ï®.J&zú?ƒk†Å">¡?c"UÊÇ?î?]Ò©l2˵?/õ€ë?PcHœ?îòTþr(?'بA4û ?†›I2~ z?F|"Ô­ú?–g»"#Ì?‹ËQ²A?î»Óº@œí?‰5E9΋q?C䆓á«x?7ëkaŸ'?£ó2E°4ý?‰óØéágAGN3FGL J0651.3+4014@eýÓX"@1­ _À:«õ¼°À;ËÌ%ÝàÀlæ.D@ø{
bZ@õþ€y0¿ÕOÌÔâùh¿éùIЃ'¿Åš—ùäæ¿Ünf¶©†AGNbcu?ïûþÉÒ¥?:°
Â)!>?\`•çû/?
Bµ	r5?;ò˜"ºƒ?9՘‹výÕ?ï'j‡?•dNç¢CÀ?k<¼NG/?kxÂÊ"Š?"© <Žæ2?">{5·d3?ï<×]?áú¿üO?ƒP'&¶ÖG?x1¯›}»=?–W¤ÙH8?Š,€y}"?ïåæÿ}ú?gª{nTT>ÎjbNB/å>݃¤LÍÃ?jf-Ö,ë?g3Çá‹5?ïýªs9;>?1[o­ÊZõ?
îrB7Úg?
º[[Ñ?.3š"]Q?0"B˜*áa?ïÜ¥¢2ç«?yì'ÓíS†?ULíð/Í?S•;tÍíÁ?h³æÎ3á?w·Oů?îæl×??š	ê¤
ú?x Wg0Âì?r¬Ô°V)™?5܇Š5i?š
Úy¬Àó?ïü™$v#?9=|é¾Ò>«'ö|ãoÉ>´'#ÓǓ??ít¡ƒ'F?97xšBD—AGN3FGL J0652.0-4808@pQ?´‰À3ÀÆ3¡îÀ:iñxôÀ;×PÁ¹sT?êº°‰íw@
üxŒØ@Z"`Ÿ§ü¿ëœ†ÀŠ/¿æf1ýþóæ¿ÝBÛB—f?œ^yæ~'EAGNbcu?ï–Ì˲?ˆfÌĒŒL?b±ùF]ú?d¥q(‹3?… .,§î?†:…±'?ïr'1>´?©š½AO¼½?'¶e¾ð?™#«ÛÚi•?•öˆA‰`‡?Ÿ™u'6Š2?í>xŒ6bE?ŸæEˆ?£$Ì_«?–oɊ¤¾?©S6]à?'†ŒF€à?îÀŽåØÙÃ?›¸zî#WË?qÁ¸U@?FÿŒËQŽ?¡ÖYnfG?™+û¸E÷É?ïÎÍ+}˜m?t
I¸6cþ?W®Å¾'Ý?WñÊhéû?r­¸ðôÁ?pŠÌõ®Ð?ï©£éô?"Mö0ˆú?k¯òÅއ¼?ƒ¿ˆR*	?}V}—ZÒ?"¦{ž>Ár?îí.ÆßDk?ŽÓ""__\?_>ow=?…DôˆV,?'ûÞÈÃk?"c¼™Í?ï¼jnU?š?|Mg"Ñ
?i˜'óÉÅ?u~õÐ¥?u;|º‡2?o¼3gUAGN3FGL J0653.6+2817@gqXf€@)Ú'ÿ"ŠoÀ9£/…(ÉÀ;¶ÄnYyï¿þK_§…jŽ@èžd"@ÿâ'…¤¿è\Žab'¿ã55¬E¿ÐuÛӔ«ã¿éå¡9ËþœAGNbcu?ïq´€Ù7?¸ˆh‰ã5r?™n(ôã8Á?¸'âjJ?m¥2ËK?p¨÷5y/&?îòÁ™µ@?£ÉîEúR?vBë®d?tí)g»?œ+íº^7?¢v®š'L?íöDRÈØT?›Ñxö9lX?Ÿ9'닼¨?'·…G:Ë? ÿ&Ú=o?Ÿ¤êhe°??֕à?ˆöm;4?4¼x˜¬4]?@ÙÙµ<ªO?Œ8Ì<h—í?‡²­õmÁ)?î_VÜI†K?ɹP	=ýx?©œ·IAJ?ɾf'ž<Z?Kv¼kÓ¯ê?Oû."¦ze?ï¸!NP½T?ƒ| 5?`cò±å?YS""ˆ‡?{î¦æÝí?èA4,L?ïRñ£´?N	²¸!æ?… ¹fT?y"py2›‡?…£7ÂÀÙ?qÆqý¿ý?ïêÌåKsÇ?]Ë[_VŸ?êãòR­"?ºkSÆe"?d×oùØ?]±–[8ÅJAGN3FGL J0654.4+4514@efŠá'6@3cS`Ð$pÀ8ºp©¶À;Vä'Ë÷»?ì²*3Uö@Vn=Í@L_ß¹Ž'¿á#±¿å0ŸZ"á¿ã[ù¥óÅ	¿æ¶ÿNAGNFSRQ?ïý1òŸ?*^Tÿô²?'¸…·l?!XÞð'$7?'UªÎ5Õã?Ù¼óÿn?ï·£W³p/?Í°ö£"?kX³ò̖?kïrô-Ø?v 'ã«Ùá?|ªu{|?ïJ‹Í<×?"
8VøN?²7MËà?r×±lFÄ?‹«9Õ¨'?P}5}ÂÑ?ïøØÍûº»?TL›éï«>ýå¼ðÃfe?å—†¯š?K­›-$Þ?TЉi¦…?ïþveëtá?y'?Ê®W1»?ü' &F?i.ÃÁ"@?vِ䕉?ï彉Û-?gVšúmJ?UÂÀ­MaM?Qý¶ÌÐZ?`
â
 *n?b9þ˜'¯?~.rô?wI¿×¦[?tÛ^öP?círÈî?~d¬o7¯ê?rµÝ8Rt?ïþ¼
k?3KÜÿÞÐH>åªõ½½'
>ò—<¾?"䂼ü¡ÿ?3NˆUAGN3FGL J0654.4+5042@d¶êá‹@5w ÈÍdÀ8Þˆò'À;y\*£A¹?öŒ¬KMl@<³µ¥?ü¢õ°pÌ¿Õj=p£×
¿àËp¶÷M¿âmX•dοæþŽÆÚ
AGNfsrq?ï÷j_Ô?D(ê'_ƒ?@¨}vC?:›kåOGƒ?A®ªu?8S©î(Ùo?r>‹×?ŽT÷¢:1g?tåx\‹…Õ?qž(H@Z?áçMÅóL?ŠRdXLë?íÌ}ÏþI?¡fó逾?£ìÌÙx[û?˜¬ÒT\'?ž£öèå?"–tŽ+Ù ?ïl¯ËàÐ?ŒàuÇO??på5œž?ptèþû3?Œar-;nã?Šà)W ]?ïüYuoÌI?0š;^(?1öN{»º?'è‹ZL}?&|$'?§æqõ´?ïÔòã.Z~?r	9lº?a"]¡%¯?WãjIÕ?ix¿
¼¿?mPùê¡´?»@™‰?•62Bå†?šz¢J§Ÿë?'.8Ï3Â?‹(;‰ß?'M>%jv?ïӁ{?pB"Lþ?eà"$»?WÎÕ×µ¤?g!Þí£Ám?kT㍪·AGN3FGL J0654.5+0926@i›``þG™@é‹@•À9ÁÃèø|~À;]²_c<æ?ÔS~"|ñ@þP
.'@S©"Ð\¿à"Câ¶v¨¿ê-ûL&¿êÝQõk&•¿ïÿcÚ½GÁAGNbcu?ï1ÕÎ[˶?—¥Þð?ˆÆ]X?^Š°å¿?ŠÄ/U"BS?Š†sy«?äBŒ—}‹?Ïñ³i¬õu?ºÂPÔя?·nº%ö̵?ÑB汜½?ÉxGÏfI?êuš©–o?§c3™?¶•«™éy?œÒûUšh?µ½€XÉÓp?žEJ¾¾aè?áÁbvuZÔ?´åwB]›Ý?Éy=Hh'?²DùÞi?πèèâ,0?²<Oˆˆ¸?ï^úP,'?Žhý°Ê§?ycĞ˟¶?‰¦Oi݄Ï?wì¾Q+c(?z:Ҋ¹p?ìsÔ@½?Â=b˜óμ?¢Ž!·Òî?¦xP¯"?µÅP'~"ç?º¼ðêA‹?í9[Åèœ?´ª%´Ã·?ªe8w—p‡?":—ú‰Ó¼?¢¸?+UäÑ	ú?êi
úž°ô?¢F$zÔJ?³JöuŠ5?˜áýqÁt?¹l±¶\M'?›²×uu·AGN3FGL J0656.2-0323@kÊ¿ÞñßÆ£'À8NAûMØÀ:Óïµ/!V?ûÇwB¬¢á@ö{ÐÛÐ@lj
µ¼¿Þ…!vŒ6¿æÔ<k§T)¿åQÇ™8e¿í²ðF"QAGNfsrq?ëÃ^¯ÁVÖ?·oáq›å?¨Ïk%§A?©£iÀÒ²Y?µ}Tíׯ5?±º¿ÎÊnr?Älì{¤ø?Íَbj«?¶9	àP?­ðDü'f?è##n8?Í Å
vò6?æ»n) ?³"ô½?À'p{ð?¨&gGÛ¯?Đ@vßý£?­¶';6Àd?èL=)ùp?µ&"Ý3?±«ç·bA?¨:ë°µ‡?Åù}w?±¢ýEþvo?í¹˜ùZX?³,ÐB£¿?£öžRGæ?§À=*)Š˜? oÒƒH"?£Z¡£]¥"?̉$/?ÓbÂïºt?½*g²–À¡?­Ã­›»$?å8m«Ãà?Ѻr@©Z?è'G45Öj?°Ji[%z?¿÷|èw½?¦ÃCsÅ?¼_ÎáhÔï?¥r´Òö"?뺜ÝÖ?¤4¯æá@º?±˜Ñ'öZ?œ)ª½Á?°–Ñœ£
ó?›82ÀTkMIXED3FGL J0656.4+4232@eÀâ€'،@2жâ—À9¤ÛÍÐfÀ;Ÿ<zڑ±¿¨›æûÍr@=¹±¼ûô@œ3`ª¶¿áÔÒKfÜ¿èäbÉ+‹¿Éß´à5Ï	¿äúµÝ`ÝAGNbll?﯍%0ÕÐ?'þ£-?W	m֘Y?e½öÿ$?;‰1I!?€5ƒë=˜j?ïÖ±ÍÎ?¡²Ö-SU?"Ê?ó˜»?†ø0:ËÑý?'@	ìy ¹?f±¦/óñ?î˜!îMŒ6?'ùîù/q×?‰²»LÉf¤?wµ'`NM? 2I¬°ó?/pŒÙ7?í ö_Üù?œ~‰hŒþ?zzÊÄ-o¼?u¶FUÖG‰?±W‹¡ò9?š³âûJT0?ï¯
Ò¯Ž?´Œ…E¢í?€dŸVˆ?´"&ÇS·?^¿að¯é?]0	BSú?﹙œÒ;Õ?6ïìé£?k±˜cmžx?`vnüœ?uZeg;
1?}ÏEŽé?ïkVPLQE?'ËÓë1Œ?yô>ê˜-?lnÀi'"?ˆcq¿_üÀ?€FÀê҂€?ïh{[fÓ?wՊ"
µ
?p'ë0¯3?[´¨@‹îY?Í3‰v4/?tàHöÛwAGN3FGL J0658.3-5832@pË¿ƒ8.À6…rÀ:cþtŖÀ;×~ßÙïË¿ûa
Œ±@`Ï«¤^@7(`Ff¿ëM:£óm¿ÎK6Ù ¿ë÷"Èú&Å¿Ô;aSñ³{AGNbcu?÷ëo¶?ˆ¥>ØÎ?:šÏ‡cÍ?…ÊÍÐ@!?qBÎQU^?lû#=ñùê?ïP…¨å¬?žEœ8Ò¦Î?v.µs·:?X$»=†³?b¡éQñB?"
x´_'?ìÄ¡š"T?¡þ/9aG?¤l§^ç^?'Î$ $K"?¯I?A¼ìc?˜ÅuYb5Ä?ïSÊƞpª?%9'¡A?O›K»Œ?[p
E™*t?"ïx½V?Œ îò@?ïÚ<Yw•Ž?t#ÔzÓ÷2?d©Zò1è³?qGè͍Ã?aK¨n?[R¶¶2?ïËD
Fã?wÏśò6®?Z惷"u?Y¹÷™êK]?s¤vÏÝÞ?s NÚ!¬Ë?¿PH©?Œ›Cb8M?'«É3ù?" ìÊT›?•ý~ÿ#Ð?'?K&'cŒ?ïãÏE«Žl?`¢škž(?^YIˆ?À¥7&ŸG?k¨qÉìª?`†-†îí™AGN3FGL J0658.6+0636@iûg_ö	Ý@_ú D®†À9¤Ï©öÞïÀ;Y#)гâ¿ÝËY'¡@ãA¯¢Åg@ØeêV ¿èí¯½¿¶¿âî`<Î	¿çq¥õ¢"¿Ý'ô)¢AGNbcu?íµm¡)l?¬`§Ëæ'Ó?™3–?—M	—/;j?¨˜ß–pH?§N9óçyé?è€!?Àµ?ÏkPN)·<?Ÿ>å–I?£Óϐ?Êö½rM?̶ôL²O?êÍU¤)óø?©]‹D˜ë‡?ªÎ›¦[–K?"Nêd[uý?¼.'•?¤|r+ìlû?ì3¶Ý'?¤M†@|§?ƒ8ÝðuCZ?%Ü`þ?»û-TÄIé?£à(§ÇP?ïfÑA•eq?–*Yq•¬k?vˆ–ª
ß?}Eúu#…þ?‹¥Þð.?'$L ¼y?íí½nq3?» »6w`_?"›÷¾ø?Œªjfá?«ýgÿD?¸®s$Í°F?îeÔ¾'SX?'¬e˜Ñ?"ál)?€b #ë{f?Ÿ*æQèÜ?‰ö"Å?ïê¯œ÷?'†ÉɒN¯?dó'ØË®v?UUÊ?/}®òëF?'$¨°R¸žAGN3FGL J0659.5+1414@i"‰€²B@ oNó[À8I?>Ú0cÀ;_ÆÞ?ÿä+mìí@ëäj"^@
ùٕˆ¿äÛUiú¿ìZi}že¿ì­Tcuv¿ï5IçÙ"PSRPSR?¿¹üN?º^kkïù^?â9J¢Ì¯W?ÎWDȺw?ӟ*·'Ò?ˍyM§[W?ŒT¤`á±?°µkºÿ?êÓ)/y??ÅÆÕDž?Âòjüè?ºæ2ü¨?Ù}¥/œG?°ýLtt\x?ØÞä"1¯?²5S‹!đ?ËHŠd?°Fé"%?Ô×w™?{™Eº3?îI_"t¢¥?¦i¡|Ž‡G?¢ÿ›
šÔ%?£]{y"J?°µqBζÑ?±9ŒY8W?êTçX>Z"?Ããe"`M%?¼£Sþ@Ž?¾ìº˜Ô?ž"Kƒ*$?½ub"Ú#3?ê ìùàMª?Ä\{\}ëy?Á©Ë p'?»ç‡x¯¿ ?Ûõj{3Ž?±V`"M+?Ù¼G—Kê?±»©ì{}u?Ĝœ°qĶ?¬HÉñ›Ñ?¯uÐ}›?¡C[ûL"·?í$a*´¬?©Xù'? (,hð'ª? NA]k¶ŸMIXED3FGL J0700.0+1709@hÏ_¿ƒ8.@#. ÿê[~À9O7¢KðÀ;}x–ê'°?îÕÇOèÔ@8Ej˜O@Ÿ 䨿刻®tü¿ê"m/¥¬¿å
îޚž¿ïÿœ¹šÒAGNbcu?í<!ƒTÖ?²¡éô¸¿ž?¦h}=©"ö?¥ÍC(‡?¥Õjäðà?¥ÖqîÞ.D?Ý)m
´'Ô?Ê<[®…³?ӏB³XÝg?Á†L¢gjë?Ύ ƒåõŠ?ÆàñG?é7ý†ÂÁ?°s[-×?À"‹ Úì?¨SxÂÇUä?µܱŒ3?žl"Í)Ÿÿ?à/ÄV±"?µ»¥Ä0'?ÔZqX»`œ?´•8§_¥?Ǝ®=.x}?­
âÜLªO?îçÉɞUQ?Ÿ 6ˆ%ž?"8-$6§?'æ¸<d7Í?aEvT?'ÍšLþӉ?奖î՜e?Å	ÂZœÈg?ÇDP©ˆ?¸]E©5 §?Â%S›!rÛ?½NVòÑø?ìáIÌÛC?¡|Óò"JA?°$ýŒÒ?˜ý¥ÛçßÝ?¡¡h³`?Žöá8ã£?èt"¹Z ª?¤x-r°ÊÙ?ÆH˜RÐ:?¡»ü›Ì˜­?¯•Sç?–Õÿ~å^AGN3FGL J0700.2+1304@iFÜ¿ôw6@kóæAÀ:6±n¢u
À;œÃT~–?ù?å{Íß@Bs`õ¹*?üഀz¹°¿ïÿ¦´	\u?ïþî j¿Î¿âhµw+ì©¿Ü2qÞrDAGNbcu?ïÚY‹©—?p2ߛD‹?IÏãFEà³?BꖃÕ"W?o2úŒ¤A×?nBg1Œ?êԐð ?ÆÇ—ëÕ¸?ªyaaad?±[DËS?¼ÇÉá=¦?Á>¿ÿð÷¶?íøšӈÿ?–ЬÜ0\?'zsʹ2w?|̄À~Ð?§¹%Ÿþ‹×?"§y"ìÿ?é'fwòï?»óÄcܖ?Ğê.ç?º_	Ìm½"?«
ïÇlž`?¥]Q™ï"?ïǫ́Ò?UïèÑRR?3PYbƒ ?/Òüôvnó?Ua!
"ä?TR&´»Ü?îd«¬?³À€ê‡Y?©º@"ó?š²eys·Ç?¡ke…"È?¬&¥"½?ï&Å•µ×?"èŽ1L!m?½sŽN)1?pÄ	wR'ä?'H£"jb"?5ãW£ãô?î\â‡QÌ?"xíµL=ö? wiøO4?="J÷?"tÛ*Oã,?‡ÐB{=VAGN3FGL J0700.3-6310@q`4óþÀ7	õ`iÍ#À:nߋrÀ;é}ü…!?ÖIÀ'*€÷@pL'8?ÿåÎÿ'r¿ìÃû"­Ãê¿ÎOÀêb×2¿Ô@¿©´Õñ¿çb=üAGNbcu?ïúfi|¬Š?@%©»{"?.^}ÇnF?.½ zpç<?=k^¥
è?7©D_)n?ï2¯Í?ó×j²?~µ€a¤T?{v¾238§?—ÑÎm.B?šWʜdÝÍ?ïä³Q[?…j‡Óáy?ˆ1'*¨zQ?}¦º•mà
?Š¨‡jb?zóQˆî,—?ïsͤ…}?PÑ\\*?uBÛ4<?n‹ˆ'ÀÌ?–ÀÕkÙw=?Š®,
<ë?ïû[Ó1ã?gIÌuHà?3jq£ðí?g?¸b>±ê?2üõné?*äÌÞþK?﵊ƒ| ã?#ÚQ"
?dÁsÇß½i?\ŒO'Ó?zÚ~L·?zÀÁ%ϝb?ï"yðíú€?x¬Òr/s?zƒ$±ÄÂ?uFÿÅ|ß??{¿jnŸÏ ?gR°CW­6?ﯳȀ?h'"ÆZê ?i©yCpž?Usd]\?qÓiWà!J?b4i‡aÂkAGN3FGL J0700.6-6610@qL>_·¼À7¿F uÁMÀ8Á¯bYÀ;"–ÇWB?òâz뮏@ìéÄTXG@ˆì |··¿×zFm!Áq¿â.ƒç^Q"¿áˆYeµ¿åôbèØqAGNbll?ïöx XX9?GÓå*¨†4?4.Iw>ç!?-4ä¡ÿ?LZ§Ï¬Z?CÈ猐?îoV؇t?±'I4Á¥?'=o l‰¦?"üaš7?¦JR¿­Žö?®MM"²?îÛÓ-—›?t	í2« ?–VJ¾[—?B›%ÍÔf?£·¿×¼'?—1RdO*£?ê£JI3'?®ÒiÂ,?¡C	?÷æ?–…q(A?Á"šõAê?®%ùú,h?ïüT''>ç?0'$´Cüî?%q≍3
?^þØ?2¥ÕMp"?%Õ¦špõ…?ï"7^!Y¨?Ÿn¸Œn?£©ÈzÕw?~"b«˜`?'ç?U/¦D?™DÈ«Ôy?ï%#ƒ›^?'ó%'ïª?Œ®ê¤ÿ?"_:Þ(Ò?'0:®?ˆ…*þ" {?î[
±ˆ=?•'t^í8?—,ÉïÊ>?€Ú"Tðü?¤T?°?"äŒÌ~AGN3FGL J0701.4-4634@p®ŸðË°À1»yß¿î˜À8®àŸ°4À;aš>G?ö—b˜ì@wëb<á@''afÍ?¿âDuÖ¤o"¿äH†¿éuE£'¿¿ïÿ‹TÌ#ôAGNfsrq?ï¥0 Ü¯?ŸµB;E?€Kîã.*?}|¾m"¨?iÌË«Õ¨^?e''
Œ?ïPL"`Ó2?"»²Õ*?w{{Y'8œ?}-ÄJ{…ÿ?Žš• ™?Ÿg‡û@æ?êÅíéÄ?«c5X¢9™?ÂeÄf2?§ØØ\?§z
Ú<4?•þ-þýã?k¥·×?‹Ox}$¼?m´X9Až?v+³¦åÕ?†gÏ"½Ê?‡NT]
®@?ïÐJ«Ó`˜?r_™QÏó?ržàˆDøM?oڛèŒo‡?Tï&ß]£?O¦ë7V8ˆ?ï·ò'OOI?~â™èFï?cç\3ŸL1?b&}Kéæ?z> L%È?xT'<sŒ?ì°m§^i?¡Ì§ûì{è?´<$2¢/8?Ÿ˜yÃlO)?™ºNÌÀ?ˆµ֙í6?ïã
;/Š?oD¯€5mi?Yä%Tànv?_}M"ýh?_ï¿ÆÌÿ?gú*˪ÌAGN3FGL J0702.7-1952@lþ"Àh¡À#j ñÀ9aLF)¯ýÀ;Cä6uÝÓ?ÔcÍ,̚V@…©Îðéb@€ã?ëÓ¿å°p#¿ÐBÜtœ¿à~8iE`¿çb,žª¶´AGNbll?ï¦ê:¤tG?…ÃJFu?gµ•RÖõA?fôk°¨Øê?€Xófß?">¾úJ¸?èé?µ*Lb?ˤŠÄÀ§?£°¯dûåç?¢ÙËiɒô?ÇnÕQ;íþ?Èl‡	@'å?î©FØ#š?‡hu§zl?'*ó¸bÌB?ƒ|r~æýˆ?˜¬1J˜l?"шWÙ®þ?ì`ú²Y?žV"é+?•êíQÛ?"lÐ{«?·˜…v»·ë?œ2e‰ÅÝ?ïä[}îÝ?eÏÙ
?Qƒsÿÿ?O«•ô"´t?bÁ8úßc	?bI)\¢DÇ?íö±Ô'­±?´iO±M}R?ŽÒô.:¥î?"	-vð—?¨à%ªj"w?°sMÂþT?ï|5ˆÖ†h?€(… ·qÑ?€MeÍi?{ZÌÄZ2µ?€¥8!¨?ljãÌä6Û?êJi¹?ƒlYlpR6?†'v‡OÛ?myt68ñ@?ÿ§qqÒî?Ÿ•"÷AGN3FGL J0703.4-3914@o;¶m
JÀ-;@Î&iÀ9›Wò/\åÀ;˜ôs®N?ð¹$y\@hó
¤×@M®€0'î¿Þqèa¿äphÈÁ¿ä­™<Ý¿êÂx‹%AGNbcu?ìh"Û"Üc?³]©Á×f´?¹në+Ûƨ?²|·€à:=?Šgo®lB&?"¬³bÿÔ?êãOÐ͸Z?ÁCTÑÇ(?°‹ŽÆBIE?«=zÍ»/"?¸Yò³½çj?º¦ùßæ–?éB
ÚÅD)?±âފ™?æÒᨕÐ?®¯QÒ/¸)?­CÖÊu±<?•8ÝÛכw?èI{Û(ìD?¨øïCo@?½CÕ¢"? 5v`WÏ?À8ƒK¼c?¤#[ÿª
?îúy§O©?˜ž÷ûŠó?›•0ð"†?–C¿›wD?tœ'êBý?oö®?gwÊ?íø
ñìR4?±gu]ŽÌB?˜i,1Õ?"åJö]?¤J—O}ÆÉ?«ÌÕ}—Ó?î5åªP?›€Á¨Î¸,?¥p][Îþ?–ªK!úAH?"¬j?¯5€t?ì×îñ†?'RŒ®"jš?°©T:Ôb?'±«ï˜?¡/dßWÞ?Š\ÌMÒçAGN3FGL J0706.1-4849@p4Ó_ôöÀ1ËóÀVœÅÀ9ob–PÀ;rd­(—?¨	,eÃç@qHA¸1@K¹ÆÄË¿Ý°¨vM±†¿çÖ?#P'¿ä¡‹^ $k¿çzÌìF(AGNbcu?ï¸üðDåÒ?zf8ãA"?qÅ,\æÉ?r
Á·?qñÂÇ-° ?lÂW¿3Ðö?îjTÔåí?³F©V¬Þ;?xÛ´Iè?Ž.ɹie?§Û#ñ"Ž±?±ÞM5o?íìÛ¾Wï?–¶ðQ|Ã?™úÀ¥÷öÇ?†à}?®²?¤4ãÊZг?Ÿˆ#®
£?ë|íeëäŒ?ž¾U¼u?'…¥mx®†?€Xh¿N?¿·+vŒŠy?Í…Ïû9ù?ïî%q‰"?\/2«úsg?Qì÷Ea€?S­§ñ0¼?QÈ&ŽKë?N![G$š?ïwâ`n?•µµt·G?qÊáÓ(¸Y?pyrÚ(…#?‰!ö÷x?'z{çÅ4?ïN»Ü(y5?~pK¯èMÏ?ƒ÷<ßËÎ?r…›å>'Â?ˆYÌCå?qx…zÓ?îÃaC_Â?'ìlö³†?{ÏəÎ$?bL&? Oòš\z9?€æ	€wAGN3FGL J0706.5+3744@fo•_x5œ@2ý¾?kOÚÀ9ºgozâÀ;Zˆ
%ð¿òےîÔ @ùó×'ĕ?þ= }Îã¿Øü½¦û=4¿ß£îX_¿àc§wÜ8¿Ñ-3FuҌAGNbll?ïÛ?pé!?kpVê|9?aºûn>Ú®?]h¹Àìõ?c6Ճò?bÄfLòp?ï‰l:ïGÕ?'c¡Íá
?r¿0g0ý­?pL¹®g}?"EY/?ïð/«ÓÔ?îg0Æqhù?•­uYùd"?"åÉRVÕs?ˆ¼xí+?ž4ÚT¡w?Žž³[wû?álcx?šŠÒwÓ?GöËhCt?McÔ«ÎËÔ?¦õV¹ã¦?™Å3•¡?ïóNõ90+?T_@ô¯?I²§ª^‹?EIba¨?Iƒøªñ?Já FÎL²?ïդ̈F?tAüÞL?\Fciâ.?TNŠZá?l8,'xk?q."¹
^?ïF†Òlžå?"³±ºûþŽ?†€C
D+ì?{È"¾zàU?‡ÞeRŠÔ?zžP"\!?ï©Äč­?sƒ=	g\,?# à軥?YKfÏÚ?…BKIÂ{A?smR\!ø¦AGN3FGL J0707.0+7741@a¦°)(@;H¡€èTÀ8監À;—³%]?èð¬Q}l@ø×è3Û@k_\1¿àd€Ý't¿ß÷ÿ`GéN¿ÞÎö ˆ¿åÆ9¤€AAGNbll?ïýEJ.nË?'ÔgCjNi?!Z΂\Ç?ŒMepµ<?*QBº,ón?"ãpG?ï•&à¿rò?‡fÄɄ?v.eõ!‡"?rD©»ÅOj?>)®"›`?ƒ™ê¾Ï"õ?ï…ß+ãÍ^?u‹2p¼ñ?xRyõ¼f—?kú'Ô7{?'^øMý"?jêd`õ\½?ïg'Ÿ`Î?‹0?Í;?o¨ŸTQ?hº–¶IÚ?ŽqnD'Ä?ˆ¹JŽ®)?ïþ¼ê4D^?@‹[Ï"i?Æ3f†˜ü?ða¸¯ü?œŒ<´ê°?qÓ 5?ïБ+G<¼?qÓ¬_Ðè>?d@3ÊþXš?X§$gkž?k. øë¨?n¶d-	¤?ïº××Ü?dOå©»n?n"%"½~?UWƒ€ò¾'?sª¿ro'?\·"Rz )?ïÛ1øܱX?jýN¢âÝ?]NcÉØ?I‰PŠ'Ôå?f&Õ®}m?g±z›°ÏAGN3FGL J0707.2+6101@chy?ò^W@9a°,XÀ:aÆÄuÀ;ú'ÌÍ£Œ¿Ü+¹†ã­@`B_A@o Ÿ1ß¿çH©`['¿êB;ԗqv¿áEC#XØ¿ïÿ¤TÕç AGNbll?ïø—Ò€Q/?H¬ç\™Îá?*s
ÿ¯n?'«7.;?Fü™³ê6?FvK(ó	Š?îÈu,Û^?£ÛF½G¬?™«nZ?')ûöâ?–¾Eïz+'?œñ"»[ÎA?î	uäLŠ?–W;¿ãt?œ¬v¯Î~?…
(ŠÔ(
?¡'h÷?ð ñºˆv?îŒØby"? gÁ¾?–œæ–|¢¡?'_Ñ©=?¢è¿/uük?˜RIŠáÎ?ïü/±™Ä?8¥Â»úü~?#¾wFßzC? 'ÂŒ?4£:i…¸?3"FW®>«?ïŒzu£+z?†=1¡Æ?|à¶Á(?s®EÁ¶ßG?|âoZÞú?€šþBŒ?îòùÙí"?ƒ+"ݝN?'ðԙîÂ?wCkoN¿C?_àRu¹?x'ÂihÍ?ï­äµ[Þ?sÑ ®Ë(ä?p[nãÒë§?c¥BåÅÒ?x²6fÍù?nª•dà2AGN3FGL J0708.9+2239@hHtÿ†]}@+•³rì‡À9ñÅíhNÀ;²$€€Ä?áo'èƒP@$Êû¼Nz@œ¬_nû`¿"C2jòxi¿à'–6Hø~¿Üa=Yt1ø¿éR6u Ø,AGNbcu?îËËþEÀ©?­mÙx1?D愛ë	?¨'Ž`Ì
¿?'ƒ3m?ƒ?'v\ p?í¼û±šJ?²M[cL,^?–Ü`I´?'JÍ·6?©*²
Z?¯«Ô·?íʳÛ3Ô?¡º5¡pªA?¦,°ç?œ>ÄßÛ ?š¥D|ï…X?ŒÙü‰sžÃ?ìö×#ùë?¢S Úä9;? NÂWiM•?Œ$áGv?°(½–Z?žæÒy¸g`?m§Å¤?žŠy/¿?Hl~¤õ?¥bg¸§Ð?qÝ\¬I5?;P@½½ï?ï:QÇGþ?˜¿PŽo¯?;(즐‡?w7ÓgØ?aL ??"+a)QV?ïŠ95?-v©×3Á?"DÁ¤E\:?‹ï\@^/?"°Z%ej=?y–HEÜà™?ï˜oU«â?‰Šéä›Ý?¹qüÄØ?qÚ҈öK³?Šç9<µß?zEvkHAGN3FGL J0709.7-0256@k4œÆø@ß
ÿÇöÏÀ8JoÛZ.JÀ;³¦‹¤?ÜM$ñ|²@õ(‹k@‰û Iáö¿àÌTw%¦X¿çŒðw]ê¿á5pËL͗¿ç+óÀÎßAGNbll?ïë"	{˜–?dÛ
¯[ÏÁ?CÆÊøáъ?F¿žK`U?^ô‡Ñß?c†é×]>0?íG‡n–-?ÁK­¦Iˆé?Øø* Í?Wu²´¬?³ˆxãÃ=À?À5 HIðº?í¦H—Qˆ?œJr©"©?•ñ®ÐÚÅÖ?ŠBÞÅõL†?ª¢Ÿ5A£?•hð1ëZc?ïf${y6ç?ŠÕ顱Ð?G@Œ;îJ<?ON9|µÔ\?'l4Qn?‰™¾¶t÷?ïùŒé‡îv?C™tƒ-ýâ?2ï%é÷?2êEhï»?@Èâ9†ž!?<²IŸA­¤?ï}PãØq?–öúÓa}?d3óXBy?hp?Ôéh?‹žÊvdï?•ÊåòÇ?ï7ÈÄ)?ƒ:T3î?…1!{žÞ‡?{µ3âz?"`v&;¾?†åPûeԀ?ïÛQ@J¯?g;<c('?9µ]ˆÞî³?2'^®r?p¼
b½?f·…jÔAGN3FGL J0710.3+5908@c¬|àü.º@9h~_o×À9ržJßÀ;ljÌ&´ ?Àæºòã?‰@ŽfÇ4?ú"—!U<¿ãÌÂó	¿Þ1ãAÙ>J¿ØK«"ÛÙI¿"r¦›N"AGNbll?ïïÓ Y.ù?UGÎb.Œp?I(ø®ûÛ´?AùÚì/¬?SÄCÍäï?O¯"ð?ï°	õ&®?†‰¬#¥o½?o€ñµ@y?o,fjä¬?x:Œª[%p?''+±Wç?ï!¶ôüÊI?‡àIiF
Ø?‡Ào`#ðå?~I9j¾ê~?ÑÓjøPÇ? ÛìG4÷?ï@f`µ?Œ%ðH¾'?I\…J_¯þ?Suì}+£Â?—2ϧÂI?‹ð30
vÒ?ïùśL™ƒ?@+dÔoÜØ?8VBIê¬?3
¥ï²r?9|䕤Y?41.£Ä¯?ïáã֏Õ\?gUd'€äD?Xô"XoÚ»?SªÂ›¤ko?a¢>sVÜ?bDÕùm~?ï"cs†¤8?xJžNª?y?"ǜٌ?púí[âx¶?}Á| .E?o€Ó{)ø?ïØþyB60?c{û™«ò"?9Pd}Y"?4kjÈö?që½3—Ô?bëþч=AGN3FGL J0710.5+4732@e8·€4mÆ@6¹Z`ž¦IÀ9mM!À;ÅÉTrH?àÊö8ßx)@ùcãÔP@.0¿æ_p¿åÙLJœ¸¿èR¶ú0:ä¿èhn±í'¿íaœÊrøAGNbll?ïö;9¥¾?M)½Ÿ<?LÉ­ª;?HOqYԂ>?5êCø©"†?3ã<œÍé?îЭ@Wx?£À•¢bB?'°¾(Ž!h?ˆS.ºÎS¨?"9žÖF'•? {õú K?îü‰ŠÐŠ?‰\V&¯¡?'³¿Ý–ð?ƒg–·Cý÷?‹v˜¶'–?}yɁwd?íd›Rh?¢²Oðn—¬?¢µúÏô²`?+1¥ ?¤CÃfV''?ŸGâÛl?ïõƒ^].?Q1"jêP_?Q¼ÛnJh]?PtØ$ñ?)ãB'iY>?"ð)f7?ï
Sr^?‡kùÓ_ê?|l¹q-ó?qҎqä(?|
TUVÅ?'¯` <œ?ïSFO´b?X‹èòy?‹¤[ÔO?{:Ò3Êúé? '¤'r?oI§ðE·?ïtÓ1ss?ƒJkI×?"$*8,&?l¿Ÿwß÷€?}\ә‰m?…a˜g:°AGN3FGL J0712.2-6436@q7µ ÝDÀ6*Ð`Ö­À: ²÷8±!À;ÀÀ//˜t¿ûpœ 4=t@£×‹Ê@î¤ûÍ¿Þ{&ëø¿áŠ¡EZ¿æÀ'30ë¿ïÿ§9.8¼AGNbcu?î¯zü z? úÌ8£¶?š÷k–Wï?œƒŠgLÆ?
Ù6fÎ?‰AÏrs+?îµ-~›ð?©Ø
YÕqR?†\U7â;ì?B+å?ž0ϲƒ–?¥¦Qa<H?êIV'«5E?¨»L§ærí?¾1Iµ<?¤c-«A´A?¯]˜x¼'3?"XƒxÉ0?î)·À\…?£Ú3î"Ý?~»Åo²?Ž;F%?©ØHµå?¡…KO{ìŸ?ïwši*ïu?µ9É"?ƒAÈáրG?…÷¸˜>N?}¯9£k¨»?yec@õô"?ï­ª³w…?†(ðµ?gE¡)šÖ?fOüp2?}£¥Nø?ƒHz#}?í.æ¤h?˜ïQŸø?¯3¸ÊN|Â?•l3–¼¼?›×±'¹Ï?'u+¦yr?ï"fcƒªf?"fp¼´÷?A»^&?E•QW4"?‰ÊFµœ¬?"AO(¥Ç@AGN3FGL J0712.6+5033@dÖN wm@7Ûß 'áÀ8èpwa`mÀ;‰þÚf"¿Á<¹Ä²L@F›'{@ºÿÅÈw¿à¯âFdF¿ãE4oØ!¿ßÐñ­Šoä¿âa°¤ÊAGNbll?ïûê2v?5Bé8¹ôÒ?º²µÝI:?Ú#¹Ý|?9@VèΈB?2´ô·ÅEg?ïšöqê?ŒT?&­›?s¦ÊZvƒ?oÐtIÅp3?O²{+<?ˆ0Û3$Â?ïO"°¦s?"¡›ÿLV?=őþÈ?x‡ž;â%Ç?‹9¹—ãLp?}àÆ
àÓ?ï;[rž?'êëÊ'§?]®idé}Î?UÊhIº'?–ÂíôçRr?Œ·ÜppåÍ?ïþ{ùEý?F s÷ç¦?ªÍÀ®¹â?¢à¡¥i?ò6<»(@?ÏàTçþ?ïÙkXé{.?oÛ~E¤?_¬vE*?Uì¶jn?f¾¤ìK?j)ôW¹?ï«$çHp?t{|°"DÀ?sÍé×Ú?q#"«Š‡)?v Ü¸?e"Ê5'æÑ?ïÖE¯6¹Ð?hd5[Aõ7?Dc*ùåÔ?5Ôµ'21}?rPÈE,ȟ?gúX-œAGN3FGL J0713.9+1933@hµ«`kz¢@+/¨þ'j÷À8EìòÝÎÀ;=xmži?÷/Oxä@]‰2C@é¨Ì'jP¿Ü	E"¿å]Xë? ¿åð9cy¿èÓ~XHAGNfsrq@?*DæÔ?´"´oú2?_úÄ?×#Ç?p‰çÀÞü?ƒVœöñˆ?´B¸Ö-›?ïi˜8g?š.šNºé?qøª©Ü?'KI¡@?ŒÂ¶EË?—W3ÍÊ¿?îWô5Úq?š
whÀ~x?™èIbÇ?
ÿ`⇹?›ñ",rNÒ?'c±dÃLf?ïÒ'½çµ9?yï7H¸Ð?=,`í¼$?Q†[û.¯?u`õFg:?yU&»g2?ïxjPs'?¼Wü@WÞä?t\¥<i? âØlù|?‡·+Þ|¸è?·h˜ÔN€©?ïÏñPÔr¢?v¦Æ|Ë]"?[òD\!¨??[ĝ=
Ã?q
ƘÛL¥?scã{Ú?ï&Ê¡îc?‰ëöúß?Žò«ˆÎS?'Éï0O­*?ˆ4‡e`õ?‹ÁÚÅz?ï÷zf^¿å?T#cÊس?0™É(ß/?6ö6šCà?Iɂ¶èzò?RrH*P!AGN3FGL J0718.7-4319@oݝ`˜À+Iä ()À8L· "À:ó>FŒ¬K?óL"=@
 wŒSŠí?ýÜ<ŒAí¿Ñ]n€;N¶¿ØÀ¸æÕ¦T¿Øo'§9À¿Þ7F¢?ŸAAGNbll?Ü­¾1Üúu?ÉBéð¨/?¯•+s'?§zÎ\¬Ä¾?ß_œlKœz?Ê-{‰´?å ÞCº?ÑÈ	Þ>ÿ?É
ãîQÓ?ȁDýϾ?ƒœ­È?Áÿ¼€y?åyÃz`Ø?³Ñ[Íx?¹ùCïý~?¡rNµÅŸ?ÍPÁã?°ÝÆ=Ö>)?җ
e÷´5?´ˆba4}?Êu*ґˆ?»™¨:ϽK?à8ÂØñã?»{ó҆[`?䈍"QL¾?Ç3'½W8÷?­~Là±?£ñä0X?Ó?sÎÙÂ?Æ-#¤ŸÝ?ê¿Ÿ£Ú÷?ÊÔ겊#?¹µ>3J
?½¨ž[Ù?µäíÇA"5?½ÂLî[?êiÒsÀ/?©å
Pïˆ?²lç',Uù?šHk§äx?ºD"å鏌?¤ˆåy8r…?Ýö$ΰ@"?²VAÖ??͒êCçF²?¯ýÐOä?Ó@f\?°‹ÇáwöÿMIXED3FGL J0719.3+3307@g!A?ÐÐh@3Ú¡–'õÀ7•æLГÀ:õ-Iå&`?ù÷ë|eV@i1kÝɟ?ÿº*áU¿Þ=eÊå
¿âdàé©Q¿ãŸ.×·j¿åqî—YAGNfsrq?ïó3©Ù5n?Qh(ùÂzï?C#Ôåir7?COˆe¸æ?PÂT_f
?H¬yŠ§T?ï°Y{5DI?‰AÑyXø?q3Lâ÷{‹?'ji	?vŸõ›#®?{÷ւW"ˆ?íˁÚÏޔ?¢©Øóiÿ?¢µæƒç‡Œ?—雬dzX? 'ûÑ®D2?˜HiqÆ?ïºõBrý_?ƒ0w[Ÿ°?Nجxú?c7ARJ!?~ªI<yuê?'{§¡0E?ïø9`ã<?DeÓýIq?>o¥ÒŽ¨?8êY
¨)??Çå­6´?9Ë@e"™Þ?ïá1§S&Õ?gsy?2w?Y37"†?SƊswû?b>¿7˹Ë?aϸ‰NÀÔ?î aho?ž>ºÒƒ®?˜y·"ó¼?"u,ýº?"z'…ÍVW?'¼gT?ïï÷wF?]–¤?=œi­??=Û»¶"´?X¡5îÇ?[l«Gœ–AGN3FGL J0720.0-4010@oƒT`ªdÃÀ(/&Ɖ½À9à¾H¥‹?À;~áxU|3¿Ñ—=7²¸"@l@ÓVq_i¿è^
¾Å¿æáÐæÊû¿ÑžÀ€ÊQ¿ëUS€I€@AGNbcu?îç@ûëÙ?šÖWÀؗ?ƒÃ¿@ÊÛé?'­gŒ?™6êwç?"ÿá
í?ì[$%ψ?¶Ô'I'L? î\ù?žX,翗Z?´¯°VPlö?²ªµ'‰à?ë©xìD?¥{ØÚ?­½]7OW?—	û³=zL?³ÕŠh+(?œ9±ñaÿ?ëÎUÊ?¯(Ì]›z??<‡ÃùØ?ˆ¤´ø@'?Â#Øþš‹m?®úo–g•?ŸELˆ?††NŽ-À?u6þ>º?r%\n_«?">ÝN&¸?€ž¹5å˜â?î´y3Ê]?¡²1"frÒ?Šâ¯&
?Šm¥'Ÿß·?œmSC·e?™Ó/nUé¯?îk"gâx—?'åKMû?šN3IŽ+?ˆÄ³ßÒW?˜?_¿ÂÈô?€ë¡£"4U?îk–I÷×?'+ɤ§©M?"ò"?qQ—W	#-?¤åc4—\4?ÛaÔËÈAGN3FGL J0721.4+0404@j–À_k b@!¼@µpÀ97-m "ËÀ;tù»B`Î?à—Ô¹¼`@þeÿ¹3=@:Þ ‰ÍÊ¿ä
ˆ&ªŽ´¿çˆ¬1 ßI¿è_=Ÿ¸4¿ä-²B£AGNfsrq?ïÚ°4`|?¬iæ:·*?;V
Û§?8Ä#òº?pò%?¬kÎá=ˆ?—5ç?©1OªÎzk?€'·§Ê}s?""ͬñ?¢¡Ø s0,?¥;ŒÅŒì?î',Q[?"F— V?‹:ï#À¢¾?z6‹6ePì? Äf?·VÄÂC?îõ
©e?"Ïæ°ï9?s%pUg5z?l"à0«N?œ†'8õ'?'yžóáí?ïûåsY5s?H¡¥‰c?'Û&©Ší?%¾œ`Q$\?4æÐ(Sà˜?G`¿¹Ôg?ïˆßZ©š?eƒ /¡3?f»®VÜ´?bwh6¶"¤?ˆMj'L[?Žµ+'?ï|§Þ€ÔQ?vë±UÙ>‹?x€´ùü?cÄÍÆèb?"•ø¥>?rÜ¸€?ïÅÓ¹g?o¬‰n|Ø?]ª-ôۍÉ?Gp[ÈLì?v
‡
ìû?m#ÃOßµAGN3FGL J0721.9+7120@aÿXÿu–…@<ú€d>nÀ6F#ÿ¹‰#À:XG·N¶F?öˆö#2_#@¥É}·ç?ÿ]g1<û¿ÝX¹ÄK7ѿኸÙáïZ¿à»~úÃr¿ã§LºAGNBLL?ïíæO!GÆ?fÈ6Ÿ€6½?;õ,º°Ò&?@øŽ×ùÚ?]6_6u?d¥@¦?C?ï¼ÿºµÈú?€@=¢?âñ?mAsfÎÆð?oåv,#>ß?rßhÔ×g˜?w­ 9Oe?ìrãRÜW?©cëH8?™($©†
k?"–Ÿwî¾?¶Ü=öÃ?¦9D슗?ïÞ«("¥ä?w9²¿Šñ?õŽâà?&nI+9W?peû9v3-?w*ÏÔ??ïòãÚ°e8?aÃNQÒD®??ö˜dC®!?G.í,?R:¤cȌ?\®?Ië&A?ïäü4Ÿ¯?l)Bg?VRYÔ»2?SØ-Ŋ_&?_µ<ÚFH?fÈ©%èB?ìó \}º?¨ 8²m»?"½•0Û€?'¯UZ´ÞB?³7—Î(Ǔ?¥—3þS:a?ï÷ãT+Xý?[)sÅã7?òéd]h?×±¬¿ï?NóŒ§K¬í?Zì§!†QWAGN3FGL J0723.2-0728@kæù€õ]æ@Á¶@™MCÀ:Z`·Ð¼FÀ;‹Õ`EK¿ìKÈÀE!j@
	†Nc:b?üÅnA&:ý¿ïX9$câ~?ÃEϯ¢'Ý?´ÿ‹ïj¿Ðï‰ôÆïAGNbcu?ïÓµ÷É$Í?vB#©»ðC?A³ªjr"O?<Qªn€˜?sîŽÙ™.P?uf%÷RØ?í}Låi"\?À#FŸ)Y?9á7'áo?†k'Z%Õ?²!úÀ×ÊM?¾ºî‡eB?í¡:´ÿ#?›J­ísd?"!<ë·¬Q?'6lÐí?¬[¶=¡óœ?—…j'¹ä9?ï‹¿2'?‡¾²|Í-?&…BFk¼÷?-ñ¨âÅÊx?Œá§<ö†?‡§Ï:?ïë¿Çž?c]Ôç¹eN?29‹ÅŠ»¥?*ðK?	#l?b´¶¹Q{?b€ÛÇ6kê?ï!¥m
?¶hg#ùÐ?k.Dz<mç?~7ÿÚ¥?˜x2Ub"?´ûóŠÌƒC?îíA·ZtÁ?¸Ø_cN?†3ƒ¤µˆ?z"9¬š5t?—>I5Ù?‡ŸÜu®¥?ïãœ|DkŒ?Z®#´þ‹?"Ô\`5?DÎ2?knäéëíØ?ZV·I"SþAGN3FGL J0723.7+2050@h­O d#–@03ËÿGs\À:Ղ}ô"À;³ÌQ|ÊV?¶ê#A@ËÞ/ ¬ˆ@3i~J‰¿å8'ŽT¹¿ì2ôG"¿ÆàÊv—r3¿ã䂳E‰™AGNbcu?ïõXBØ?W«±ö
,?/NFܖè1?+-p1?Qe5¶"B?UêP±jf?ïkӂôfš?"Øš Ø0¼?xJ·c>?ƒ~mZTÁð?‰yÛpü?ò¦ïü#h?îÄ]Z#7?Ž‡Xˆß
ˆ?…/H""¶ý?s»|;9â?œÜ°jwŠT?ˆ¿!­=ª?î׺|›º?"OŒ°'$²?a¡FZ±8?f¤5?W!Þ?¡jCӄðí?"ρ²óó?ïü›²$¶?;["'T*?•;ª¿Ëv?GæY< ?4}Ó\þ¶?8FdµÀ2?ïѝ™®g\?rü®ªð?aÊ¿Ó&oŒ?Yoiqj?l—¦p³Äƒ?m"é3·ÉÐ?ï€ñMúM¨?xТÂÔ¥°?t¡Ô+"|?ac ³¤"?…rÂjHHC?vHS#f(?ïÀ
.Q?nb•é9ê?[k'hŒ?Ko'—ƒ?y áàum?k6|'ISVAGN3FGL J0724.1+2857@g² ìt2@3[½ ‡_À9¤LˆnÎëÀ;ÄŸþ7©¿îíPzì°@kDDž:@Ác `Ș¿çíí¸nŠ¼¿æu"—™[©¿äßOᔯû¿ïÿï-mnAGNfsrq?ïçþ›ÉA?kÎñö {?={àû•öº?CYÿ "F?dQè!áU?j•ÀDËÛd?ï'D+º)B?‹)±"y?r–%¦¨'?m"µqoc¥?'#ìî$;A?ˆÖWRŠ?í¿5Ԓä?¡ç6];?Ÿv‡ñ¦uö?"«?­k½Ñ?¤Q^¼TØÀ?Ÿe—*öÆ?ï­ju%R?€®!ç]&?Sú%ë·÷?]'ˆPå)t?'&	àZ?Ùx1z?ïòêM'-d?b\Ó¢¢?A<‰ð6y?J¯Ñ2à«?Q <õúz?]÷}®'?ïØDÛ8Ë?qt&§6uÀ?^GcõP',?VÆ "¢y?h˜7Á›½?lHXvs*Ã?îR|êê͜?r²Iõ´¦?›[' H9?'´ˆ¬c*/?šTѕ=Ò9?"'9Íùj?ïò!nuåœ?[ÃL#!˵?#@Ïj7Ç?#²¢*N§!?YU	22÷?[\
0
ýêAGN3FGL J0725.2+1425@itXf€@+Õà0VàÀ7Z)¤>8JÀ:æWS£ì?ø|§ÎÕ@9ðh2n@ø45f¿'¿á,H›Ó¿ãàNŒ€–¿äXɒ°œ@¿åµØ[4AGNFSRQ?ïæ(~µy?e"¤…ç{?L˜éŸ^S?PÑË]
Åõ?bѝ8Ùê?bGñŒõ ?ï'4Ï%Óµ?"Þç¬wã?jYE ,«?mf+mD?"ÜzÜîl«?'ÙF±ü?îH띷$^?Ÿ"ù¾Ã*Õ?¡%ó(¡Í?šeÈã‡o
?"—Œgñš¦?ð9éy¹|?ïöñ‡}s"?^…d¨F?ìäðLN?)T'kÁ8´?Q•CYD?^5ä-³ŒË?ïñǝãÖ)?]ªºIú?K˜E}Uõº?Qn<#ìÌ ?MIAéÉ2L?TOŽ<RŒ?ïٝÙÖ[Ó?t£éL‰ïK?VïÔ|*0H?U)&é?jê<(4'?q,sg.?îñ¨€ß…Ù?•7âyÅ.?—
†Z'_Ó?'¼'n¼q?…€ÓJñ?•Èµ®%¬?ïþ®zëóG?2ß",é¿G>ç…Q"é|ì>òÌYÍ/
[?#ŸøjùµÆ?2ŒüœnÂAGN3FGL J0725.8-0054@k69Àëíú@òÆÖ¤èÀ9EG1í¹À;kÛ._"?»ÍÌçyÌJ@%–¸Öq@'-ÈÈ0¿ä(›	—j¿äŠÔ˯ýo¿Ù+²ÔÍ]¿âr»7½ËAAGNbcu?ïš@7	?'ÿ5"¡=›?^µéGã¶?Ußjh'?…™?>ŸÇ?êÖ'µjÌ?ì	EdÜ¿?Á@´´A!?•ÇïVÍ]?˜‰×t`?ºDãéZ2?¾­/§Ò0S?ítð˜ü? Hï›C?˜Èz€Êw?…¶ÓL~ïÛ?¬Lø—†
?™¶
?쬶NR–?¢U$äT"?‹'ä¸^¨B?ÎN֟'ë?¼0]¸9dG?¡'ÒK¢üÖ?ïãjʒúˆ?hgl¡a?M¤.5Þp?DƗ•´Þ?e,*Ðkn?eÙðD ÁË?îí³]Ä?¦+Áß<?€eá'ez?…HêL
S?š)ìg»³Ç?¡²é1=ï?ï/±n«?…Úb"qW?…áKÐ12?wµç:o¼?Ž2¢'¿?{GxÊJA?îár$¤hï?Ñ}F3ä\?{®-M^¹9?b8ŸãC‰}?œæ0ßtÌ?€q\¸%¼AGN3FGL J0726.6-4727@p6B 6mÀ,;ý!(n´À8Æ¡ëw²¿À;TwÓv4:?ðMó=yÞ@"rYä¢×@¶- t"§¿â¿:pœÔ¿æÃÅð˜7¿çù=TZ†¿îK7ÛRelAGNfsrq?ïÐ7uä?pVtÀ,[?m•¬°ý|?f|ŸºzL¾?b2Þv-ÞÔ?^›2ÈB?é–7Ww?Äðì;Òê?µ±«(û0i?°œm¶Bl?½óßØÝ?¿xíD!Ô?í®¸´´I–?šïüÍ|'P?¦́òk¿?"üüän^j?žNj¹_Ç?‹ø¡¾‹~i?æ"Ì°:V?¯Ò‹ð'í?Á¼«y?§.yìÔIÜ?Ãô´TR_?¬KR°CW­?ïۛõÇöW?hÓÄw»Ì?jç'Ý
ÒØ?dÐç9»²¦?RùÄß8üH?NêÈnù¥?íGŽ®²?³lìÓË?¤_Š(]MU?š_ü\4óÍ?ªküö‡Ç?¬¼ùœÃØx?îµ
€Xø6?Ša"üüŒÐ?š©Ð]k?ƒŠÓ–µœ?k$IW?wúúQQ@¹?ìf[ˆß.œ?—"a6£@'?°q¾ß'Z?ŽÝ&ê®Ô?¨¶É°V­2?"§˜þAGN3FGL J0728.0+4828@e2;o@9ÍÕߛªÀ:‹"äþòºÀ;çú#G-¿ú›yhKÃÎ@ÒÍ`Æ@÷ýÀ4¸ï¿êÞÜKðÄN¿à§ê{ož¿ÝDTî™Ñ¿ê<ߕ:AGNbcu?î²=3+p?¤E>­Íž¨?¢¶)ŠL{'?£†t¯ƒ?q0(*?q¸v§oѺ?ï†çȦ¢l?—J ¼XJ?w×dÿ~½Û?€1fš‹?'Z[GÑ´>?'MÈ>@ü?ì‡=?¢PâCø‰?¬1ÆŽÄ?˜Ó¢ðS'?«}öK²l5?–ëØ'_D¨?ïubÚ¸P?…j͊T/Â?TçN—Õ?Z)ÁpÖ]k?3¥Ü¹x?"Yyqǟ½?ï©´þX?'0$ö-"?'ý­wjmN?6SÆs
á?Uô‰5e•ñ?T‰œãm?ïÙGlP5M?q*—ÓýµÑ?`&´X7}³?[Á]4èÚ¿?f'߀΅€?iô­è¹Bþ?î"EºÄH?'ÕÀÍvQ&?šØ(áгð?Œ¾ÆTÀí?'¿5÷‹?ÂÅhÂ?ïæBw§_?^½êMeŠ[?) %¯jiV?']§îv‹½?h#…Ú4ÀW?^%¥Ñ©•AGN3FGL J0729.5-3127@n¢å>‰©Àŵ ÝDÀ9´I窞¥À;Q¸Æ…Šï¿ë=iöqi'@–'%†ø,@;µ¿j
»¿ãô§¾6-¿êˆØ‰C‹¿í
ÎÖü¿~ǁfûjMAGNbcu?ïufz]i?Ãº""²|?õ§‡þò{?‹¨Kmyœ?€Æ~ޑ/?'ÝBÊÚ¡"?ìæԙä†í?Àh"Ôbî7?ÖѵBQ?•Sìýsþ?µ€ø€2T?½3‹ó"¶?í´àÇÖn? 'Fš,âB?žØˆÇÙ*Ñ?‹œÔÒù¹I?°46È8õ\?›u¶ü?îòŒ|¶Æ?—¡‡Tø_?7J™±Û'­?F%®@ɔ? °âVž?—Œ‰u°?ïËÃ,~Ó?vTê¶ÀP?bý;®B¥A?f&#ü8¿?pþpó?pGÎSh:…?îæĖX­§?®ˆb@3¬?yTÅa™)?…ÎÏ)Øß?œÒ;ÖدÓ?ª»ç†¾?îÖû
Yt?Œ:S…Z"Ã?À‰IQJ?"#0ý?•@Z{0(æ?"|¾ÙUX?ïÌy}ï3?pÌUþï¸?ÁÂ/TÑ?YzÄ?y|:1?p¶8kdÛAGN3FGL J0729.7-1448@lÍòà\̊?øb½ßôò±À9¾hêÀ;[Sã¬ã?ÖeäJþè@ÜÕô=Ôø@\›`C™¿à±ùĞøK¿èÄxãáo¿ç¿ûö¹Ž¿×L¤•ÃPSRPSR?ç&D+—Í+?Î{ñÏ ö+?ŽR…!×/?'I—±^Ÿ?ÐÀãÁ¬2?Íè˜*ë;?̤Çcñ?ÎcõÈÄ?°¶L/Õñê?¬fñ~¦Ý?æäÍH
2?ÎW¾UÄ5W?é!׺«Pë?±LG‡L;Í?¦UTR4!½?'v¿Ïä.h?ÅãKÿ²Ó'?®ä™ '´¸?ã8"f=s?¼p'Á]O^?žM¸ÎÞ0? ·üxd?שý¦ÀØ?¼lClˆ·?ì^ÑæÿÜ?ľ5'*†ß?tœº'gº?(,7µ?»È[™ž?ÄLÓd¸Þ¦?ÞJÏÒ:Ê×?Ôg'ë­7±?­‹H骈?¦cmZó×Ù?ÞÌDÞù—?Òöñ5Õ?íº1ˆHí?šbŠcÿ?•>ïÚæ7?ƒi'u3?©½ëìúI?•ïÆË ½I?곝`où¯?¨f/PMëÞ?"TC¿–…?‡ìÌ]?¯Ÿõÿ 1?§ƒÆäúMIXED3FGL J0730.2-1141@lxl_9K{@	Ø_ÒùbÀ6b²<'ÎÀ:l)±ª1—?ø'{j×@m^ÒsTá@¸Æ§Þ¿áapD­üJ¿äǜԷ|Ù¿äç|×I±¿æ£#$a"AGNfsrq?ï;бïâã?•%gqÒ?VVkÄ7?T[悮Û?— ‰'"_G?"¿ˆ~"¹d?îq°æ±?¹6V9ñ³ú?v4ò˜ëÌ%?"÷",ºvž?¦SA	yj?¸m¡€*Î?êH[@˜v"?­ŽêL'ÿ?©·Ê2ô?œIn'•_?À›‹PŒ³?©9ÊâGûp?ïšâšû¤?Œ€-¡Ø??eiå
?Pwõčš$?ˆL0_bHò?ŒBÍ	i"?ïÑòÑ÷·?yžFB'Ät?R¾}ÿ5?TJm"ö¼?rWMG	?wO—€ÜQ¯?ï}ւá¤Ô?¥Çe¼"½´?b‰´6ºdˆ?sI'Wm
?‹çò@osæ?£ƒ…ÊɁ-?ì©B^tT'?§0PG¬ð?ŸÖ%ƒJ·Y?"ÿ–äãç?²Àc¬Ôˆ#?¢®v©ã:c?ïㆤÁ¸>?qM+‰'?36"Rp?=ÜÔöŽþ?j˜0ªl!?pȒ,? AGN3FGL J0730.3+6720@b'ºKâ@<™åàš	+À:Xg`ai§À;þÓôß:Ž¿â<žüÚ܅@¤­'ÊÈf@ëø :G¥¿éÆB+ôz'¿äòíVkWοèˆ(»`å¿ïÿl³Ì9™AGNfsrq?ï㦐xÏ?s<~èëŸÌ?c܏õn?qŠ_åLÜ6?Pú¸À?S4yþ¤Û?îÏ·ýv§–?¡:È]9\'?"œÑÛ g?'(ì`w'?'l.lóõæ?š7ZÐn?í6ےý?¡i=ïny?¦Éè['…¦?'Ñÿ©¨a\?¥È^xè;l?—»S¾Ÿ?î}ò&×
?Ÿ€gÆ8ò?œ{~}=Ö@?•2Ë
ÂÑÅ? ªaœ_ï?"9»/
;?ïî"£?ZJ&­Ôe#?XæÚØdÄ?V>ƒ"³Ô–?C&,C[ëÎ?@SƒX²ee?﨣ڇ—Ü?ƒæ¡|Âia?tºFgŒcù?pv‹(èÙ?vóÌLhž-?/Š…Pt?î¢\ÿ½îk?H©ð‡o©?š¥ë²L5?ƒÑ¤£éù¶?'¯º°®n?ƒ}C¶"Õ?ï³
ãºÇ^?u/ª þ–â?ls*2CJ3?dȬ$Ô?x?xè~l?q¥°ú¡ñAGN3FGL J0730.5+3307@g;öÿ:Þ"@6e>‰©À9ù>
ÈÂÀ;̐"£¶¿îvº8—îk@2ˆá:˜@ïý |¢=?ÍØ¢òŽ0¿è䴲Ϡ'¿ßÆNdMBº¿ÓŒÓ
‡ #AGNbll?ïˆZEàxÀ?›ð×½'f?U¹èìU?Zp"[RR?‹97NãÍK?šÙÖýP˜â?ïžP;L?Œ?	D??r¶aG5þ?pY)U#Ÿ?~Ò'ð¾µ?ˆ†2îñŽ?ʌ½?'èÁòi™–?ŽÀ±UŸÌ?}Áö¤	Q?¼SÝ쒌?ŒJ‡#%?ï(ˆV?®?d€Î•¦z?E‡\BÄ,õ?G3iy?šBºX¹§?1ÇÛóǓ?ïkðãqBÒ?ºÖ¨¥€P?]w!'¢›H?"pÐO˳µ?ªqm@?¸väü@N?ï܃Á–ò?p¡ñ_6?[Ü£\û~r?W'žzr?eì'9þÔ?j7A¨o?ïl—ÙâM?|æ…̈́Ò?Q³ñÈ{x?p× B'³F?…1/"d¢÷?tÂ<ôOº'?ïÛɵK?f>«8Û?#?'xOõ?&~ÃEð?q)ZN;?eò†kN¸ŒAGN3FGL J0730.5-0537@kÍóFí$@C·À AÀ9ÃÁð8À;Šf¿àîð…†	@Ä:ø‰@Í쟥ø"¿æSñÜѧ¨¿ä´Ä16ž¿ÅÇ$%hA¿êèˆ±ò´AGNbcu?ìùƒKpä?³wŠ{†˜'?ž!uùn{?˜]sò—Áæ?°« †úƒà?²Qž…^µ?솕½/å?¾œ¯‰×?'í~Iç<«?'`LÛu¾?·Oò'½)Ú?»î"Ølh3?뤛Ü(?§Û2Þ?³ŸQ|dú? >;°ø^?¯³Wð—?š9›{GÔ?í¿E†ƒ"›?¡éé>þ?t,Yaà?uOq¼ªY?°Å¥F
? ˆ#@#!?ï#å"Œ¥s?™r/¿?ƒ¸9ñ×?}¿¾\?'úŠ=)?–s‡z›8?ïåB˒Ì?¢à>¹?v.Ú¯µ‹?u¶	ÊØ£"?™— ù'Ü? 'ŽÓ+±k?î)ÊÍ)z?˜ùg@ž.=?¡dëç?"?3Ü ]á?˜rËÆà?ˆºásë½?ïd•x͜+?|#]úp?bnˆ+¯œ•?Uqæå?'܋ ?yîA꘩AGN3FGL J0730.5-6606@qZhŸÆÚEÀ4Õ  0øÀ9ÑwÛðuÀ;‡±ñ\Ï¿ï;¹ñöw@
»7
³Fê?ü 4á368¿éÇO á¿Ø´–×ꯃ¿Á! ]FñÆ¿Ý8úÉpˆAGNbcu?ïÂÎtþÀÌ?xÞ©ÎÅ?I/çûÐû?E½òö°?{räuù=?w¸?sŽ5?ïl݉¦?…inY?qZ³ú˽?~2ÖÀŽJ?ŒC¶	Ó?‰ïÂ-'#²?î6²ö{¶ž?"¾ÔŒjÏ/?âÊ£'q?}mãÐÜë?¤#k…ƒ8ä?Öì"ð?ïN›Õš7?ŽA0¶|
?5ð'Â]â?@Ùãæ?ž>kêl—n?Ö½–—ê??ïåæÊW…+?d~bœI¦?;¡¢ÌqI?7ý_2
¢Á?f¥sžæf?cH
ð›Ì`?ïÏÛ¢¨‹û?sf0ÃçªÚ?XzYC…iK?Tt­/a?qó˜UYHP?pX†)Qis?ï_H;bš?yZ…1­¢?~ô©Î½?fJ"­?ˆíöã؟A?q£ûúb3]?ïÃskBÕN?gÖj±TñQ?(
ná0¶?–ß™ê‰?}…Þø…¤¥?gì²»AGN3FGL J0732.2-4638@p0Ã?…Q
À)ÌG¢'vÀ9e¾/áoÀ;làæ_E
?úÜÐ*zR@šWÍ|2@)ë‰%ƒ¿Ø8qÂKOÆ¿æ¶É ûì(¿îýØP
´t¿ïýïmqٝAGNbcu?î§]¥*?«ˆ~po'?–¾ä¢nŽÛ?¡<µÉ<Ÿ?"UzaÄ5ç?ž9;R>û¹?æ<Í\%&?Êè4(É?Ã<?î¤Û?½´/$¹Pw?ÃýŽO}ZŽ?Àë´eðJ?ä°/š¿è?´l	·…?Êwaò?¯à&S£W?ÂÇâ¢w
Ó?ª:õkÉÊ?àcógkI$?¾âØtB>‹?Ö¬µHT`2?ÁDĞ2¹?ÁÇѪ?³\ž"à_?ïN,ʨ?¢Ñ›ýÑ?Žãݧ¾ßõ?œÑÆÕ¾˜?{.m?ó<A1 !?ë 0eè+?ÀR'MÒÏ?³¥­=n?°ñ$‰»ïÊ?³Yv¶7+ˆ?³èª%$t ?æ^Å
"66?´O"€?É
ÃÀ'4~?®ÙÔIÓ9¢?ºîP*9åT?©Sߞ]9?çç%ÀÔç?¯^×»P>?ʖêA¸¾?¬(@ZËîú?§1úú·µœ?˜˜JV<AGN3FGL J0733.5+5153@dÀm ‹]@;Vš ¨4À:pÚ7›À;×5Ú­` ¿ÏÐqûxf@
dÈÚ#øX?ûÚß?ãýb"Rf?èòKÅXí¶¿ã¬[ñ"׿½7'lÃf‹AGNbcu?ïÓP.8?rŽºÑvM?SÈ;AAbO?Q]0èxJ?qeÚ
3>?p0~/(_6?ï`Ç_ÇÞ?%óÂu
?€`>§?‹G¡È—?‡n
ÿ»ð-?—w-fž"H?<:?õåYgx«?"pŸfÀ²?…YpíO?™e¢af?†u:[ôÝ?îÂ<¿½´p? \qY¯Tß?' èÛZ¶?™ÉXkTvu?•+6î?"Iòy8<?ïôÊ´ž?S¢Å"þ?6‹d¢¨…Ý?4.Uœª#?RQ'µ¥þ?PöÊïÌY÷?ïÖJìQ;K?uZ%Öubn?bŸ"¯Lx?_ÙãðW¦è?gñäP²?qQÃÂ)"?ïWx«sœì?'}nۑÌ?ƒòÍY
?w›,8'š³?†/ڈÚ×?vÒb¦¤?ïÑX»`œV?päé#ô"¦?Z—€êT'?RW
%çPø?p­ÛöVx#?m¯mœ2̖AGN3FGL J0733.8+5021@döè ÓI¿@;½°ŸpÀ9Å»{k±)À;Òîî_Č¿ñ§fiœ@îKAFò-@¾ÿ¯£¿çúÚâµû¿æª¢_)Êî¿çCÑ`&Ó¡¿ã-ËÏAGNfsrq?ïþGʀ'"?!'Ÿô#î:?/3à™?>=Vïm‡?!ëÄõÜ_³?&Ùߜ§5?ï±}Qb7?ˆiñ,ÊÜ?p§`˜¥_—?ñ …2ç®?vš^õد?y"æ5çô?ïoC`857?u~
P[@?yB=ýe•·?a¶n/>L8?‡Žñàq?q/jÞ±Ù?ïÞøÇ:?j;+èÀc?
8éFöm? w$	3Š?p¿Ôü"#?iߦ
|«?ïÿ!
@Û<?(˜¾çj?,CÁç?hÒD…·!?»¥Às~h?åÿ®¦{?ïä1K®:?eôrs\
ˆ?WÀW¨ÆMÑ?S÷®vÅ4?_ÝÓi?_Æ9￲ß?ïº06˜\G?c±G@Gw?lÌ}®kâ¡?Y^%1QÛ?t¥É^?W"\Îóz¯?ïû'As£ø??gp÷Pv>ôýnÕ$6i>öÍä·Ý?B»W™ô?>©W{ɂAGN3FGL J0733.8+4108@f7)à¤&@9
ohیÀ:.ήN\"À;ê‹y¢ƒ? ¨8t¹Ûñ@
(2F#Oæ@ÆÎ`u¶¿ì˜î
V'€¿Íɉ¬¿–¿áf`­G~ø¿×¶óËØõ¿AGNbll?ïèSîaŽ?aÀ é¸?M¥m'…/é?K™–ÃMÉ?`B¶@äÆ?]4Gv1n?ïLüf(º?œ†?ä(?'Jíþºtt?ˆíž áÙÇ?Šuø"Õu?–pêŠ=L?îHEv'ë?–3s"vs?"£ƒÏÄ(,?"îgnÕõ?¡,Y½E!F?Ž®[?
Sr?îǝQñ?'Ü"Äë?†#;ž…Ÿc?vXÈ«Am?œ
¿Â:\#?Ž-[Y²?ï÷k¬vk?Iq¨çzÛ?9¯P¼.‡ß?8v%¯è"?Ey¦ÇR"¨?C!€rƒ ?ïÊ<Ìû'?}e¯ÒÙ?e¢9Wàë?f·h•g?pÔÌ"»?wœ™ÌïÛ8?ïZa½àæ?|¹ˆ?[·ð?Áa¯~zˆ?r—øÉÂ?‡¦.Ïâ†?qޙr"1z?ïÁZ™ÿp?o=ЙU¿	?hjÅׁY?XT|¹£ø?s>L[Ã3=?h1"¤û¶AGN3FGL J0734.3-7709@rŽ¿ìºÀ8(àÉÙÓÀ8аô)2À;n`TÔn?é"tþžoÜ@H50cu@R'ıJ¿Õâ°)åù¿æHû*‹¿åðûDU¿çq$Ê(œpAGNbcu?ïúpñè?<ݧÝ
í;?9÷‡ÉA|6?6‹^—¥;
?5Dù+þ"¾?)xyçÕä?ïÌÇ»¸?Ÿß^$˜o?ü¦âµõÎ?|Ð0o4œd?—Ýܬ£=†?[Ž–è+¦?î !NŠ?œ`Ü)Z?"
=Ñâò?…©R§Ë>5?"±¾UEÌ?€âW¢|>?îü¢'‡®? dgÐÍ!+?"%ب2n©?zj* Qš?ªæ¿²Êýq?ŸPD®¹D?ïüõË?*èÞv•?*®àÃØK³?$Óæ2ô?%ôrþ¹"?n2÷7‹W?yÞ	Ø?‡éXöE©ô?iŠ$?PÖ?e¾Ê>Ø?²Áĕ©?"Fdòצ*?ïNÍÙoÐü?‡¬þÒã¥?ˆi823tp?ƒYÿ[-Ù?ƒãQgán¥?x;Prò°?ï}«4A1?Þ¿hã$Ç?sDB©å˜?aŽ-ùº ?‡±Ì<ð?€ g‡W[‰AGN3FGL J0734.7-1558@mž@ÈG,@ž 'ðÙÀ7⥤i×4À:÷ì^òÕ@™ãC0×8@²ß¢<€d@"fx/º¿ÖÒXbËt¿ãAVÊŔ'¿è%n+¬¬¿íì¹®€PSRPSR?QB¤,'Þ?_ˆºXëÑb?ï£.§CŒƒ?"¦qÅõU?…¥xsO?'yù¢5"
?6kMm—Þ¡?XÃCüw?ë¨|6C?´O©AŸ‹?ÁRف;(ö?´"eT€{_?ž4ÒÌipI?':9FN—2?ìAgŸ‡«?£4öV?¶j¸
Ã¥?Ÿ¢q<TÛT?btä€(7?_%6
Hf?îÛe¹9¿a?"!oÿPßj?¡"V&‰Hí?"F3ïZf4?HJä]Æï?_aޚBa?ïu}žÍqI?¦}˜]䟘?û=¾öw?¥µW\ªD?SZÆ69Î?j7í,•Á'?ëœö›Â?¯ ¼Ÿ>Zj?Áhú™¨vñ?¯•¬R˜y?­ys3~\§?Ÿ"¡#¡|?ë÷èè>ö¾?¥"ir¯?±ƒÿ#Û(:?œN#	Ö?w-¼™«d¬?fØÖ c"?îĜˆrý?Ž\¥§¬ÈD? ÐâGå?‹V*´'$PSR3FGL J0738.1+1741@i;dÀßXÁ@2'ŸªTÓÀ7"^™éJ²À:ÅD1ˆ8H?äëWÒNí@yéØ÷'"@
?·¥ô¿Ü3†Ç¿áÏ-à8¿Þñë²7—"¿Ü»ã"$VAGNbll?ïùΚyµÆ?B­$Σü?+Á¤Ò·[?$"q"¡Ù?B¥ÄØ@Á??ï·F9¶?ïz'¬\Ï?–ÄÃWÙ??w]_؈çÎ?v0ÏÉ1ð?…°¤÷;xa?'Å`ÓǖA?îÝ6¬0íU?™0bÚ{ó'?€í$ÃEDò?€ˆM²Š‰?›â˜,î?•ß>ôšaº?ìÉö]…R?¥u€ÓßE?u…jњ½â?r$™Ð"±C?¸Wø†c?¥{G$$ú?ïýv—zÊ:?&‹‰[{'ã?ÎÜ£Áa®?a£ˆò?,/LIÓ?"¢ÃškÿÊ?ïÂ;Ÿhf?ƒì–Ï'2?e	4}pN?cF?b="O?t;Þ#˄ù?€¤9ˆr?ïg‹y"×?‰ö""ÚÝÁ?t¿ÀÞ9£?tÊü[m…?‹½Yb(†?†…X'Q÷?îóG'JPí?ˆô4·ñ?l
"	Pìñ?\gÑÊiö?ž]Z/=´?‡ïR¸3fAGN3FGL J0739.4+0137@kËßÒc@&е~ÒmöÀ8%W¨]'À;T»ÉoJ;?û$G%Ž@>«6z@ SMÚÔL¿á𗳡"Ê¿è\·€à:=¿çËíSÕë¿ìÆ©C'ŒAGNfsrq?îp>=tÍ?©
xnâÈ?¤ôÁˆvÁ?§«rz	ì?€(j<"Ç×?'gû©éz?í¼#n
)?´I~ƒ
?–~o´d?•='äw?©<	åiÎ;?±ŽÇAhBC?ì*cì8¢ß?¨&üùMNá?´±dr¡?¢å
qÕ?£öøWZ¨ð?˜^+^œ{H?íd…ÙÁ?«¬ïükµ?¥j²ÓáÅ×? ¾ë&˜à?©/Tœ…?¦Çmã}d?ï
Q+…"?Ö¦Äjã?™XÝy³Ä??›ZõËÇßÀ?j.Ã8Vº?qՁI¿-Q?îòëQóÛ?Ÿó~MÒ?ˆœe`]áþ?‰d9Že5?•Tc×Í®?™9¾×Z‰'?íB6*Í?¢rŽÔùÔÞ?®Õgt/1.?ž^­ÃÚG?špîñ?'Ê¡é
9?ïó¬›»?ŽóþÁ›Ô"?'›6Ñäû?ƒyÔÆ®4?'âï{.?"ÒèÓe-±AGN3FGL J0740.8+6621@b¶°À&Ì@=œzߚ.ëÀ:frû À<Àu¦uJ?õ»½ ´ëÛ@7[íçy¡@1Ø@žUÁ¿æ]¢ÿ/0Ö¿Ñ~"´Ç6O¿æ½"e¹ú¿ïÿïÝÚ!…PSRPSR?Þa*쁌Ì?΁œ(Pg]?ß
‹þ?Oe?γ•#SÀ?¤ŠH§eiy?ªÍÁå†?Íôæë˯Z?Å-9Y›…?åmQ?˜?È\Ÿà|ú?»2ǟޤˆ?·³'âGÄ?ßÈ«›à×Ø?¹I³HßpR?ØâÔj>Ñç?·å«¦\W?½QÿçY?¨ûX—ÄøÛ?ÙȖg
%H?·j®ÚgwÛ?âs`ù•?·nêÐ/? ÄÀ—Òs?˜‹ÂË©þ?ád"±QÀ?Љ½Íš@ø?ی@
>3?Ðu¨Ìp9?š©i/tï? Ž&­j'+?ޏÂi¶@Þ?È.TÖ_âX?ܑÓƪãˆ?Ç\)Ê\bµ?³y§=1"ë?«â™2ƒš[?æ9ÐZ9Ì?±
*È¢é?Î5;‰v"e?®Õ1Ït¶¥?±ÇŽPò?œ·Ò¸ËÃJ?çdZ÷Ò?­qKÌÑI?Ð}àLþ­½?«ÀÖºÛ_?‡-R|,Sú?†mÖ¹MIXED3FGL J0742.4-8133c@r]…À3aVÀ8ù_{šÀ:ÃÃX¯Ä~À;»‰'ä™r¿°º"ËZ…@	Ü=IaÕ?÷l?¸ý¿ì‡/ÆäwܿٓtvŸn›¿àÁM<ɵ?Ø2E-¹AGNbcu ?ïݳo·%¤?nL¬..U?7Þ[4Ÿ?6U$~Yô»?oPÅ3×'?mŸ0wæV?ïlšÖc,(?•Œ ¨Åh?qšL0ªù±?ƒÀ2ðû"É?Œ$HA;?ŽEž"rú?îOÙc«my?•'¡ËŠ?–oJãJ?áõfl??Ÿ•ˆ Ÿˆ¡?‹\ÿ»,S?îö|Xõ?œþ4ý!y?PÊN»újˆ?b!àmpX? ½vÔe?›Ü;Í5?ïåüîŸý®?e)â^Oݶ?,_¼H±?'ýפÁáõ?h=KÆç(?d¼•5ço?ïÐÇvTM¾?y¦Ü%lås?Záv¦C?dÒËkCˆ?pë\ŒÍH=?p§Ý8{?îìØ¿Z"—?"â&ºÏ«A?'i<[ZV©?"ZÛÛÂæ?÷Wrª,ê?ƒ}º
ØÔ?ïÑ&;†œo?p]ʈ]µ?5í(sÀ|?Bö6³Ò$?v¯?ß?p0‡4!Ò±AGN3FGL J0742.6+5444@dam¿‹›ª@=Œ`Ëò²À7ÅÐÂû'³À;3ÁÑÇ'?÷¿n2†@È8'ŸT@(ªªŽ—¿áV£Ðª'¿ãôIL
€É¿äŸ&ãæç"¿èU)ßÕòAGNfsrq?ïöÎ݌ýC?I"Ž7?Fbz;Õ
?Dãu'i?<Äásm¬?5Ø#‹W
?ï¾®Í5?~'"¾Y4)?lŽßž?nb™Z‹
#?r¢Q'&µJ?tç¦ÛŠŽ?ï2é9+è?ŒäÙç?‹C$5ø"?…_v9–?ˆ™É{oÉ?€ûôŸ'7?ïúò³JÆ?U¸%3âÏ>þû;UÙÀ?K(‰c1?C?ËN$´s?TØg†Š"?ïú·D‹†m?='À\øÞÚ?>@½Më}·?:CnÑ,K?(
;XâÏ?£U3~?ï碊Â?bÊDËKÄU?U8)¼
ã?Qå떹Wá?['ÁqN?YQÖN7Ä?ï{—Ä6?ƒÑ^BZ·?€lÌÐáV?w¢r"íÉw?€­rˆz}?|…‡î"Gx?ïÿ«êÌ_?3|UE>ï¾Å=¥Ø? ãÚ`o?q›´ ?2Ú$ª‰AGN3FGL J0742.6-5623@pÍN wmÀ/c1àLÜRÀ9Ëú/ÜfžÀ;£'ð	è·?ãmÛç-1x@7º¢Rв@n[à¦sr¿èV€G솿âM.6c¿ïþœ ::¿îŒxϨ'AGNfsrq?ì9¹{'?¹€guXgb?»â%þ±F?¸šßWÓvk?'€qO±—µ?Ž3ùÝJž?èÝz)D{?Ȇ<ì*Ç:?¸ß	mð|?´iº{ì~?À9`b°?Âò»žÒ?겝Þ;£ß?«ðŽŸ?»¶oÜ9"å?¤ÿ÷AvŠ?­iB`cN?—Ú)ÿS¨?ã2iµ·m¦?¹Êx¬¤Q?Ò=Zn`…Ò?¼&M,êªê?½wH"vø?©Gó&Y?îjïJƒºh?§•fm0–?¦Ã ëK×´?¦Cp~S~>?toS€ ÆT?{¯S½³Ô?í´õZŠ?´"†Ñˆ à?ŸO§23ƒæ? p@Õ¨?¥Ý=•?¬ž¤Ø{¢?í'NI;Ø?œ)nØ2®?«æRž¢0Ü?˜ýŽ
Å*í?—鑛̹Q?"^»ßV?ìsësšÆ.?¡ê|jq©?²Š^è°G?˜ìNŽ?£¬Œ±ñ؊?"èÓ&­ËAGN3FGL J0742.7-2824@ny)Ÿ¡—ÀÎE s'•À8àa'ÑÖøÀ;!º+àX›?ö¯þr·,§@C1.ãÃ@íèô>׿Ò&'Z¶°¿äíî/ýW¿êàŧ‹í¿ïL3íÙPSRPSR?Ë7^'õˆ?Âb¬×}Ė?æ;<²ôð"?ÆÇ^	0çe?··]D(ÎÖ?³y¨/?ŽÒ§Z·"?™ò›=Â?à0éZo?ÃÕ,¤›!Ñ?Þ©`ó&]?ÄAÑSÀ?×iܨ#$?¶ÌÓêT?ÜÀ}e¨È®?¸˜#Àj?Ç«Kâpfß?©" µ­üq?Ã_"?Ñ?£ˆéá3g?å,gÖud?´ü%kN¡†?ÇðØMg?®®ò&œø?Ú§¤¾T¨¾?È"=™µë?ààDSʋ?ȐIApo?¬¾"Ìf†®?¢2D%íÒ
?¥"òŠÏç?¬º¾J†"?à°¸"žœ¨?½ìþõòi?Ûû>:ß`4?À:¤´³Y?ãÄJŠgÍo?³)ÓÅܺù?ÑæüúÎ#?±86ß,yD?ºA·Á‰
? eé,N?ֆ?]ˆ¶?§JÇêöQ?àh'–ÇØ?¬›"'ë÷Ø?ÁRãt%Ž&?ž¶{rT?ÏMIXED3FGL J0744.1-3804@oŒ-@ªêûÀçÆ«±ÊÀ9®œ­JP†À;@R,†q¿£Ì0ú&@
m‡Aþ'@q³?ˆ?¿ç¼d™Ì¿æÐ9Ó$C›¿ë3@ð=ÈÁ¿ïÿ+‰/OAGNbcu?ëi/nM?¹-ӑ–?¦ÕÀèJ?¥?Uä姢?»ÑÖ&Ü?³ê/âó_?ÝBÀ!¡C?ÐÔÀ=Ç>?ƖGCzAÿ?¼³Jçý!K?מ™\ÿ?Ê+"	e7?è¦â°
ú??«Z•¨"?»Ìrù‹‹~?Ÿ$0#ä?¾üw†¢?¢e¤ÑY?ßs¢ÑžB?·ñÝ·o‡;?Èdm4XC°?·°ž
´­ù?ÔZ&"5Îæ?¶G@ÀÛ?íyù¢‡˜ª?¬ÛÀQ	? ë!™Õ??¡toÙÉ1?§uD<ÕOQ?¡Hb›ml?è¡«ÛÝÙ1?Éãžñ?³Â
"Ÿ´ˆ?²¤T)³ª?ØIÿ8Àø?Ánÿ«á³?ì•–hâ˜?Ÿ†—0_y?®²qÊÑ'®?•˜î0Ç4?§û´ÐX|×?ZsÜ8?éH‡ÐÉ?¦=˜˜»îÆ?°±ET?iÅ?™´Ú¸ÿ(?Ã6;6žú?£ÅCAGN3FGL J0744.3+7434@aˆÏÃø@=–²ß»¼ÚÀ9Êìˆ3@À;Ô=ß^ŸÉ?ًž`Ë\@Ú6n&#U?ÿÉ¾Ð_Ô¿æ
ÂmDÉU¿è¿²sð‡¿Ñ]i4'пƧrŒ¤AGNbll?ïûÞ-zë?7~ȎU¼?öqw‡&?
"+'´o?9ù'™?2ù¸™?ï­Ñ;"ÌH?‰"²;Wî?qÇuzŒÛ?ƒA
ùŽæ?wOì´l+i?zÛ{äln›?ïP‹rr?waTþŽŸ?qõŸ$+, ?k؁;ÌÛK?'ñ
°U?q}ðV¤?ïŸ'eÓ!-?ƒ+¦•ä)÷?D`'¢Cf?Q¥;¦±?†ði/_?'ŽóÂ?ïý"~¸ÓØ?(öFà-?|†SŸSš?-ä"Ÿ¼?(ùҟÿ—?"\+8ÿž?ïâûÛ-7Ç?ey¯ÔÑv}?XÀ€ŠhG?S&~.X&ã?`£ä™ò­Ñ?`¯SüÓ?ïÅÝq'Ä?kÜxD.?g~sg7?gt	¡ó:	?qQþéGg?\ÉÞmžo?ïïè2_N?Xo³÷¨Àk?9ñ:·.I?8ïá–k²?Y³¹l$á?V#"£öGÐAGN3FGL J0744.8-4028@oÑÞß)À 	ÙÀ%I'À9cý!(n´À;RZ8Zº?åä68@
h/žÿ	5@·[à{€T¿èø-®d¿Õ^Ž1퟿äC†Änž2¿ïÿž'ƒ© AGNbcu?Á8ÏC8~?¿Å¾\¾ê?èà•¬z?Åݼ3Lˆš?¹F‰³§Ê¥?¹¼C…ÄX=?´Ÿo¡—x?µåkæ>I"?âŠ`l/Û?Årœí-ŒÍ?Õå×KgÍ?Ät›"¬‡?àùS¯eÄç?´Ÿ¾ÐŒ=?ԏ;SjÐ?³çtü€?Âü;7ÂÄ?¨HUâ¾.W?ÐÉ_™\v½?µ5JDqÉò?à­@¢Ýe ?À'õªUm_?˸>?«¼‡?µ?ÑH©ß?Ò:}õú?ÉZ«¶ìT–?äî¹["\ï?ÊëÈûÜÚ·?¯C®]Ny[?«°[PSlž?Î¥ƒÎ'Zò?ÅݙKž—Ž?Þb_FÈ¢'?Ðø?ÒJÞÑî0?Àt*üNj?æŽæ3Ž´?°çÚþÀo.?Ëâš1¢—ù?®âø÷àj?³ÃšÞ ë?œÚûѬŒ?áln_¦{!?°â
~x?Ó¹°PüX?²¤.Z÷Á?ÂÚåßmc[?¤šÕ"'±ùMIXED3FGL J0746.4+2540@hWFà!q@6Ø1ôoÀ9MC%¾=À;¨¤Ô`?¿ô¨cpŒ@üç¨eÝ@¶šà@œþ¿èÎíd?οêß"Œ"Dè¿çO¢D
 ¿ïÿû
LàAGNfsrq?ïûD«-–??µÜî,#t?'J-ØZp?'m}*­ò?::_I½¦?<Q
K?¸Zà?'›¼Ça¢?x*æq…?zwRlÀdã?€ž˜SjÙ?Š9b‹·ð?î¼t"@X$?'–ÁDzУ?"tÓcbþ?ˆGþ%È,"?"ýa¦If?ˆÂWÚ°°Ï?ïVý²ó²À?'cà1¢?diqhb?lQ—™%?'"v	8ç?'@°80aá?ïü§3=͟?:£	ėôÊ?(sTàï=Y?&WéûÆÕs?-xíeœ?5UPÙ}?ï×(­+÷?r+‡®¾Ý?`lÊ5õ+¥?W¸¤X-ÎM?hjˆœâp?mx¡ªÉ½…?ïïU`¯?‹$~0ÿɜ?'Ÿ8tM @?ƒú~‹Ì&Š?‡E¹Ý+˨?èJû¡V?ïäÕ‡VÕ?gµ'DÏá?,šáç…?1+8vÍ?ijÑÊØiÛ?gŒãüßÒAGN3FGL J0746.6-0706@l6Èó#@!½•`$À9þ!ã–¹À;kfKŽt?Õ:[¬ñ@ºÁeæcÍ@‡Â yÒ?ïìkü'ƒR¿å›Üc‡}§¿â÷ˆ"¢Ø¿êøÈ¥î(AGNbcu?ïlÀ×rÇ?O|ºÇ¯?ÛbÏÂ?€Ið,®û?'ôJÍ&6'?…Âë€ÑÛ?ëƒ-JL:§?Äbw'D?¡ƒ@øv?§ð"‹ÄŒ?»%˜.‹?Ày'Ñ!E?ëˆ>C÷??¦Ñ#éQ-h?³óîó¿à? ,ó
ö"w?°.ò.+?œ‹Ï»ê{?èsõ…?´ýV¥7¹S?­,çql='?Ÿµù¤Ýu?Æè£çj Ê?³V3eΊ?ïÙ)…+¯?pû=pò?f#œÝ†Üe?cٍ7ÔJ?`²Þ®Œo?bYØÅp»i?îT¦{æf?³d4ñ9?õ'AOcg?š}lÿá,?¢¸3ôµZQ?¬k*mØCÐ?íҝqaä?›Z¿T™S[?¥k"Ee?•Ú'c"?šå#¾r­L?ljä<M?í‰ò@¾zé?™âMÍ/X?™ªYKm3?"Û™úò¸?ª‹"ÊOÏ?–¿œ¸&AGN3FGL J0746.6-4756@pUÕ`"¥À&¢ù;.ªÀ8øžâ®¶aÀ;Wƒï
iu?æüEH3 k@x¡Ú±@¾_쥿ç®(&ÃA¿äãˬfOë¿á%]èÇî¿ÖM¹º1¦AGNbcu?ïsU¡È?ž6Eì†A?s;¬b''?|qÿ[?‰ŒÏf&±?˜Æ‡r×aF?î¾áæÿæ?ªžkŸ)—?F™7Ž'œ?"–=™n?Ÿ€v‡ñ¦v?§Cƒ&TlX?î"1D	‰?'Å,\ŽÓ?'2""v_›?«»7'¤T?žGRò7·Ê?‰õ? –i?í6'eó¤Ó? àI4?uÏ_3Ï?~í‡Ú¸Éd?´TD«Áê?žÄ"'B)?ïŽÄ§Ëq¿?£·ÐQÁ² ?s*Ώ4…Ø?"ùPÐ?'¹nÆé%K?Ÿ¨²N6èÌ?ïŸ"¶™Á?ˆ¾~	Ù
F?h–ÄrþÕ?eª]jõ-?'­àƒ"?"Ùvôv?ï}x¥†?}%†ÓÀp?zUÿ®}U?ntòƒÀ?ƒw´ó-?w#‰fU}k?ïGô`d™³?€B½`'nâ?s™Ä1QÂz?cˆU¢¿u0?'ä³?}/'ÓE>#AGN3FGL J0746.9+8511@`à·ö@<. Eð¥À:/(âwYÀ;ÐÍ×°VÀaK:»è¤@ïàÚñ?ü˜ì€Fac¿é™'Xßj3¿à&ÀøÇì¿Ö8ðÐÞg¿ÍÅaðA¶AGNbcu?ïéÙgåÂg?f2M1òx{?4:yr-ÏQ?1ÑÄÔ¯U?cŸI	ñ/?e£ã(Ò?ï²ôù*'•?(¾¼çó?n˜©?6??m¹13Y–Æ?w9.ØÚ
?z"Úók?ï8ðÙ¾Å?"@tZ·û?…É»ÜuÈ?sàc1dž?"ký'ºv?}FìRŒ?ïșŒâÉ?yL$§ý>ûð˜Ê5©$?¼@2ÙÚ?{—Hë.U?y@ÈYaüb?ïø7"šÎg?LßÍçKK?&bٔ£Úa?&Záoҝ?IŠ¿LÀ""?JÙî
|r?ïå"¬lR?fÛxMS:?Wöá–Y?S[«'äuj?^Ûßì£¿?b‰L¾­ü?Á™®?q­Ø?y[@`tâ9?h=dœ?ƒ$¯Z ³]?g	E"Òï?ïö¹5Hê³?HýwËüµÎ>ÎLî Zœ>Î<N…Š›?R~nïn±½?Hõcïx5êAGN3FGL J0747.2-3311@o
•$ÝÀٟîó=À8ƒjƒ+™À:Ø G2Ä?Î,Ùx'ôö@S­|$"@y¹h¿â50hJ
¸¿æNíìW+¶¿å)‡ZID¿ä…R\Ä&5AGNbcu?串—Ú¶? ?Z³Ö?WKîN%u?U²ˆä¤´?ƒüФØ?}¡@*BÐ?킇a]½ö?¶~ì5œ×?ˆ'> 1‹?ò-R @?°ëËô/ž?´nN¤¬0ñ?ì¢On/ç?¤É'å?Ÿj5x¾ÊÚ?'—€Ö"b¶?³÷/ã!Â? r¨K­†?îsŒ'Àª?–ß%°aß?W+7ÐÓ?Z†|/Í4h?¨|râ?–HDgcœ?ïé$€à1¦?_Ì·øÛ?A\¸¯­ÿ?A¤fL"á?b"Q0è¶Ó?Z'q¥?ï8Tq`.X?šf±r¥Ð?rñ'ò·º»?s~™ <z?"9cìT?—;¶ªð…Ä?ïÁx…͵?Ž÷ù.&D?†¹¬þ^î?|GÅië¦ä?"*úqÏì?†`œÈ¯#?ïŽ1@¿¸½?w;
³?DFA¹ô$B?9ҍ*oÒ?‹/K®:v°?v§õ´ÍAGN3FGL J0747.4+0904@jb`RP/@0ˆçÖyõÀ:d%‹ªÃŽÀ;àК·§?âˆéߓ_)@Hî=à¶9@‡Â?ÖØ¿ÛB¦¿X+K¿Ó $ØÒiš¿àø°ªF(ó¿ãðsÚ AGNbll?ïޅÖæx'?f+Œæ?]ô3bgÝ?Yzu|Wä?b€JïÇ?\Ôó=Î€?í/~ÌtôZ?»4ÌGc8V?¤.د©ÝQ?¦O¬)'õ?¨Ù:ˆ*ö?³c¬£#À€?ÐعÚ?Ž.5p¾¯?'¦ĝôà?'1껥?œdý"å?ƒ¯ç•¤7D?êeÞãòû'?­ÜÜså©2?¸@Öxg?ªQ£™tF(?´úÐ? @ïduw0?ïðYˆvJ?Žd¥_r?TÀ²…ˆG?Ž[ò4´i^?F:^ía»?=%· =²h?ïW;Á±?l×íO??'
<Vy?'Ú"úæ%?ˆ1ôÉßë4?– Ó֞‹?ï`N%U?vügŽw¸?z,'eU?m(CÔ2Í(?†rLí|AZ?mE	ɤz?î!¾WØÈÈ?'–=Gð?¤c=v‰óT?ˆÜ^.AX{?"ºŠÎL?JlMñ¦|AGN3FGL J0748.0-1639@mF÷_²íþ@ÎÙãÀ9/Ã¹þ"À;CÖS^Kæ?õ–qÆì¹@ۖÛúT@Ö[ 9ÆË¿â
^¿èGCˆb\¿ì˸0F¨¿æ@ºr'(AGNbcu?ìS䡳L&?ºaà&¾':?²K"&A'"?¶¦7Ê2?¦*­›·´•?¦ôKLÆâ?ä®9x5Š•?Ñ>ItƯ?¶F³½üJ?µÃˆÞ{ïç?ÑàÃrd?Ë&fÃcm?ë7 -´?«`¬¢(?°—ïÚ\Ç? Åèãüb?µ«¹"ÃF?¡£«åMVˆ?▦ûài??¹á©ŠŸÎ	?ÌNKîÒt?½–ËQ*G°?ÉW#Ò?²ošL?ï
CÐöc?žæFªæs?"
9|".?–˜A»óG?‡g¼ÿY¤Ó?ÊHâ<¸¨?ëJoAx½£?ÆM..ð?¥P uc¬?¬×väØ?»&]¢G"?ÀA"µºô?î,Íë}3?šÜN±õÎ?œH:‰ò:?C»ÁŒ§Ä?ÖúNðeõ?'ÓãŽÄÏ?é¤SªÞ Ã?¨Ý=ËL ?À µfB˜ñ?¦­Þ»…Ô?±›÷Ù,	?—ðAGN3FGL J0748.3+2401@h'FŸ¸@6­?i¢[À9ÀÜ0À;³Ô&]aÛ¿ð ~ðËډ@[µàÏ8@@`k&¿àñðj¿ä,fꉏû¿áéñd '¿ÕÙ°"AGNfsrq?ïþ‹ÏV•?"¥¾c¯Üí?,CH|»>ÿŒb¡-©3?*</(KŽè? ±³ë€ÿ
?ï¶ñè v~?‡Œ³Ÿ!ü?oƒÀ,î!?Ü懠S5?tÅ+ÝmGÆ?wâzÎú?‡(†?só¾?ù­?t§æ£·y"?aÅ«·{œL?ƒDªãó¡Ï?m7ݧ'…?ïî{ŠÝ5?\r¨êö}¨>ì¥I¯ß»>ñ4ìو®?agÏ÷Án}?\]PšLžö?ïÿÀv?qql{É>ýÏËr<ÇÜ>öâ¦5k?J†óð?íDØÛ(¥?ïäg»˜‰?eú°5îs™?WWq¥
›L?TT§õET?_Ùf|s?`n¾¶ËäÞ?ïÅ4cΠP?`?¼9žá?g¦&"sù"?Q˜"5R"t?q'ºÏ–£?Y3ÇQÝ?ïý:þèÜ?2þus[p>Ó·ÞÚ¬¦>Ïe›5ŽÃ?5ãeäí?2ãƒJnêÿAGN3FGL J0748.5+7910@`ß2_c<æ@=GÐ@ÔÀ:›OC427À<)LqMJ?ñj®òÇ2Y@£àÒ¾(o@¿ï©H8?Ñõ%†wRó¿ãæZû#L`¿ç«Gþ‹$¦¿ïÿ¼rÙÞ¦AGNbcu?âBÃc±D?Ô²Vòތñ?Û$BÄ9š?ÔËÈYºJX?u m81³£?~Ûk-CÏ?èéGú•‡ç?¿ÛÎGv6=?ÄÕ²*kø?»=øQ='æ?®·ªÎ5³?¬eÔÌô°"?æ/_®wˆ?¶
Ô$Á½?ÍõEd89?²rRtõ¼?²2y{¡I? è}Ëew1?å#×Ñô»?¸:O¢í?ÒÜê—
"R?·Ï—6Ì?¦Û.(K<ƒ? ]¥Çžf?æøO'&=?Òovk¨V?ÑÐ&Øu¼4?Ò
(Žƒ¼?oË߁x?‡ÿ.ºK?ío~çÖWT?©¡¾&ýÖì?«á&N‡ó5?£lõãÑ´?šMÖiÜý?š¾[Dçi?ê~äü2YÞ?ªb©&À¹?Á~¡R—ôË?§.éŒé?¢*ðÂÀò?' æÖ='Ð?ìÉc°	? ¨Èävr?·nÍéoF?œ5ˆý?'0ËÀVs‰?ƒ=¡
þAGN3FGL J0748.8+4929@e$¯ÿ6¬d@=XlÿݛQÀ:3½äÒ}À;âÅû!?ևæ³þŸ®@
­ÍŸZ£»@¶jyÍv¿ÞíG€ù¿ã©;ˆAWŽ¿å¦ÐWN¿îÑzÎþ*hAGNbcu?ìo2QÙ3?¶÷£F2í¨?·‹;6P¸Ä?µÄJ#8	?"ìÈïXk?B•{Ò´B?èæF.ý2_?ÁNw~´?Ãsœ ÆDÚ?¹©M\#?±æ•IùP?³œvÓ©g?êˆ@~³˜?¦¬
Û"B?»ÖB\Ì?¡n…6
±?¯Ï{ð»ó?—YWï‡
?ç}Otîz®?²$®0?ÇÓn^yÕP?¯	ƒs¯?´n§œtfð?£àÀ?bÐâ?îoÑ}FãÐ?²«¦á{'Ž?¤ªÉMŒ1?²}‡uÚÁ?a¡"_¯?{wfa³w/?íùT¹&
?¤"ི?¤cIdB·Å?uH† {?˜ÖàWª?š"þ¡tô
?í¹×"×?›'wª?¯I$‰'´z?–C1H›{ü?žV|'D?…È|±"y?í'ì¬?—zÉž?­_"Ýõ?'5ÃaÙ?"º tU§?… FÄÐùAGN3FGL J0749.4+1059@j/
€CR@1˘<eâÀ:¬ÿiÀ;¿­Aí
?Ôpw%?C@™#îq¸)@ŸÈ_ÂX¿ç&J;¯Ðà¿Ý•tè—A¿ãVòì'Zõ¿áKâù×>AGNbcu?ïü{êÃ>?4.ZÃv?!UíÏy?W2܄•?3u±¦i2<?0sŽùø®?ïntWÉH<?•¸;öºØ?yË×]7€?ƒQÓzš‰±?‡|þpmWE?'ŠÙ§›?ïlÈë
L?T9"cQ?€Nçã4?rh‰ÉjŒ?"ÇÁï$ð¸?s›`6"f?ïSYÕoš?ˆ¬xw¹Ÿ?x+n¥ž?o'ô\Ë?™
¹DWc?‡€ˆ‡•¹z?ïþXTÍ.>?ñƬ?"탳4™?–¹åTÆ?aq¸h·†?8\:oï?ïÑ^ûãç?z6'(³ô?`fí¸"NŽ?Tßµ/h͛?n~³"M{?w•D(­®?ï¹\%«òH?måÂÃÝ°?p‰·DÁxJ?fÁuÈ¿?rÈ5æ¥;½?WÂõÈ‹•?ïÄCšù.ï?i¢+r¤T4?e)1·ãÈ?Pü±ÝCy?sI™æîNŽ?deo&ó™žAGN3FGL J0750.6+1232@jì O*à@2»`c'À9c+Hƒ'À;pClfZ¨?ë
ªj³c@VF,	HS@J:Ÿäƒ¿ÛTÌÍ+J¿éX¿Ž˜+'¿âßã鰝¿è Ü/&šZAGNfsrq?ïùjÁƒ²@?CÙPډ1?;ÝÚ|ÙK?8KIc'Úc?9›‹²vú?8ü½¹í?ïr›õ®1E?–'Nëw<4?x –ú2*?tÇÿe×Çf?‡K2@_´?"°y@Cù?îùÍî#ÎU?Š|à?47.?ŒG‡?€oÍ1:yg?'¢´÷ù3N?'P,S /?î"ÐSY?šÑ7PàSy?Q/•=m5?vèwìM?¢Ú1ë-·©?™x%KV$+?ïýBLš|1?,[*»¬ƒÞ?+'ª'›?$ã-
bf? I1…K+Ú?!"Ã|9?ïÄi
à"S?}ƒöi?f«j>ˆ?\Óǟ߬j?ru÷
ào?xŠèÀå;?ï‰
s4?|™Yh1?{{zù\)!?qÑ«¢¾X?ý´ÎxÓ?s
	"ë7?ïŸnFڅ?uΌ@óÁª?t<9º1yÖ?\ƒðcú3?|:cÃÐ?sK ËAGN3FGL J0751.2+1806@iX;o@5ÏÀ¢À9Ò»úÀ;¨•Š@`B@†äÇ@ïßq<X?ûxt=i—ô¿Ú"DPo¿ÓˏNÖÁ‡¿ã^;÷š¿ï!Õ2!oPSRPSR?ˆ¦¡|°³?ƒæ¨³@s]?ïƒÂ9ËÓ©?‡:UÿJS?i£?Ֆì‰?dóq?s'?ÐI¾kßB?¢šÿ!îJ?í>þ[N?Àx¾xø?±Óýä;?½©jÌ@y²?²@¡øç¨?¡*èdl‹û?ì
´á•þý?¥¥¤íK"?ªÓmñb<è?"@C²Ÿ^†?±Í":‰T,?ž͘ó®?ì¢Ô¡‹:?¢Ô—Ïó{k?¢7­nÍ8?'Ez4Xà?€IÝL1^?€^PµÕ…r?ï¯.cž>?ƒ– ?_ŠºžkúF?aÇ5Á%w?¤6öC5+R?³«½}Ïc«?ìMÈ¡Þ¦X?¶ >?³v?Ïp7˜?ºšŒìµ?½
Ò.>4w?¦t×%æ?êÕû§««?©R¡7›a?¨"¡*€³Ï?–Äê¤OàP?Å®Qú&Ð?¥¶}»¨É?éÚCžc®?§`9WÑ?—Dþ'i‹¼?²ø$^/PSR3FGL J0753.1+5353@d†A¿½ð'@>…Á?ÐÐhÀ9?ª¹|ðÀ;¨"?…J¿ºÆ^;Ó|@ ®÷#ã@ØúÀP»¿Ñ•º'L¿ãþ-Äx.T¿á5(²7Œ¿ß_~þ°AGNbll?ïú:Ī?<C8ùµQ?%ñg"&S? ;
}…&œ?A˜"sþ—P?8ð»pª?ïYöÊ?]Fó‹?uœÅB?q¹ïêz?k÷9z҇?‹8"B´ß?ïNnÆîLµ?…¿Ÿ4/©Þ?ƒLë‰Z"?|I9´öz?‰bÆisq?|-
U±=÷?ï"(ۆW?žq´g%?ec‹?^Qõòß%Ø?™ºy¡´?TDœoÀ?ïýᰚÎ?.T°Ð§«¶?"XÕs­Sb?ˆxa…§?,©ùÄld?%¶Ær]?ïÖÁi†P?q.ÍÌê½m?a6N»åÍ?Vƒ·´|"ã?h&_õâ×?mcEû|¸?悔Nˆ+ç?v:÷~œ~?u¯Ïl3ŒÏ?pæj}ƒU¹?uñ‰YUgÙ?iPÄË·Ô?ïÖ ü'z¢?kÈ÷MÿeD?JžÏFnƒt?9ÃÁ8•.?q›§µ–óH?j½bçJæOAGN3FGL J0754.4-1148@lÙ)¿*å@ y–ÿáL6À8¾2lcÖiÀ;CÉv7]?êÅÐsYN@—M·B÷Ì@á©`6 £¿Ø@)vý¿ãsQŒË¼¿ßMJ!G‰"¿âª¦žS¬iAGNbll?í܅9eQh?¥yÑ{}çÇ?"°vêgôM?o²äpê?¨_põRÖP?¡­z'1žé?è?t|©žÊ?ÊÖs)Bn?µL˜}óri?·Y(~¦œ?Ä[áÎÍ¿!?À§Gd?ëণÃ>.?¤AAY?¬ÐÐJŽ?˜f¾,°i?²'ÇúµPJ?œR"¤ Öñ?㸪¿9nê?±/cʆŸ¸?½ÔÐãn
0?«hÚèw?ÑvH±Ÿ ?° .Ó¼V?ïD¶"O}—?îæ_ífÐ?ƒé4ëN×ü?€a"£jC?Šé&M0ZG?†E)Ô'š?ìÏêŽ~³d?ÂP&Òw½?¤Evíø5?°¸(cTß?®€¡&ч?¶§ªç¨Mð?în«d|?•Xቕ?˜°ñ`–?‰øƒvüèr?™®ªÛ‡ç?‡Tõ¾GI?êoŸë½ö?›¶fð)<G?´Cz§[¼#?'¾é®[§Ù?¸?Œøjm.?•‹˜Žÿ"AGN3FGL J0754.8+4824@eQ4 -œñ@>(l <K
À9š0˜N@À;ž"Ž½ž?À¬ÔOß!Ÿ@!eÁzß@$=ÿêÜW¿àêø2†K¿âÏØ°ZÑ2¿âTSK×nç¿ã»´0É¡tAGNbll?ïÓØA}¬?sy¨9þÕ?^¹²r¿I?U¦ãC-¿'?mãÊÂìÜ/?pUÌ
"*Œ?î÷ëºV[4?£¥nêèmr?Ž"|R^?ŒÓ#eü,c?'ñH6vD?ŸÖGÖˁ³?î†Ùs#c1?–'¡
xÀ5?'A@Õ/?…Q*ÑîR?œãÀcšÊ•?	yñöŒk?íA¨{"!?¢ZS0?•Ì¡"öØË?‡'¬o?°"¼"wI?¡˜ÿžcá?ïõQ#;Ìè?Râl"Ñ?BeR"ä\?=lÇW÷?HVj€$/?L|0`¾Õ?ï°º´î?ƒô9¹³'?s33é³?tÇÈ	Ó@??touRû!?|<>²0Öð?ïpGõ¦Ï|?þà©Á?€Ÿ
€×åß?vD^·'??ƒNõ\•*?t¡éñ_!"?ïaüÃEË¢?*-AR?yOƵÞ('?bN†Ä×jH?ŠØëߤ¥B?öÄTô"AGN3FGL J0756.3-6433@qTR_ét£À1Â\ÀË6ËÀ9ޟð˯–À;³x«ˆ¤¿ÞtÁ' @atÇ},¦@¼T@(4¿ä"ôµ¸Î¿åM7È2"+¿ãW'Ñ_Ú¿Ù+Ҋ뚲AGNbcu?ï…G¹8Vš?‡ë×FPÛà?C}"moK?=^só²?|Ó|ž?‡´å>L…®?ï:0tæ²?œ¸x#t›«?vÑ»Ü~z?ÓA4‰3?"Ž—ó?™=¿Hí¿?îHbF""¤?'µ	È÷ë?'ÐzX'Ë?zKZë·µ@?¢'žiSÜ?ŒIrûî?î¹,ߺ™?ò–Å ?X,B~¸i?V@ ­zÇ#?£¬é&¦†2?·1E«?ïãp)VÍ?f'˜6uc?3ÑF}>¤h?/"­+èˆ?jÖì4jò?e+Änh‰?ïÃ¥e÷øí?{_O&öè>?_'—Üÿï•?\, ¬TÎ?vH§ã¦?wH/Â,	D?ïpX•öÕh?r‹ßë
A!?{Ôë`ªõk?`€…þ‡†ÿ?…ÿdâsKS?j¥˜N—œý?ïÁhÒɳ_?iu!1Ùaö?@wÖ^'Èí?1Åùbé?}<›â€/"?hçp4A
lAGN3FGL J0757.0+0956@jiʞõ#-@39 4¾NÀ8"ÕϪ͟À;W4H)?ëÇ:
V´Ü@"Ë'Rz@trŸYÌû¿ãàN#Ïh¿ã£dÃüÆ¿ãq
â秿ã´^zù_AAGNbll?ïúÃx˜Ëœ?8¨ßƒáJp?&"F,—ñ´?‡~é?>ÓyIÞö?4ü#4ýlÿ?ï]±¢=Ç?›_ïÌ"¥>?|œº986?wz¶+¬öS?Šlö{Üj0?—ÿ
µÜ2€?ïUç<("
?Tós;ù6?ƒ?·œ¡¹?v|Ç@»Åà?‡FyÙWA'?sOàL1?íëéšZV/?œQ7iÉ~V?Š¸	W}Ñ?~àïêØ'?ª»øVLï›?›ËH°vi?ïý쵇?#'IÌÁ?U·îﱩ?1ǒ½ˆ?"	КBj†?ªS¦ Ñ?︘ÄØ ?…Ï'û·,?jSE%ì¼?dèú.̞?v‰û|oµ˜?ÛG¾ú^þ?ï§|Ÿü,?mXÜïënþ?t¼‡ÈõFz?b§"úä!?w…laC·?a+"
öaô?ïrU"¹/.?|m:Y"ãú?yh¦ù›?`Í­³Z›?†¶=
Á¸?y{ÿ[¡]AGN3FGL J0758.1+1130@j=ÒàãG@3õ[_¢'À:_Y²"ý[À;ÒNér?çMÒ%U@G®¡hšô@QFt›?à‹!Ω=H¿çM>Dð[¿Ò@bÒn]'¿ëJ¥mQ+AGNfsrq?ïÌc{-&?tGV±2¬–?m5"Ë(×=?j¤CÔ.­ ?f«y‰{€?eb%ðB³Z?ìz±_ðÛ?·#/`éða?¯÷¾«áj ?©µ"ìd?¨]+Se¹µ?­(1ÃcÆ?í~¥ã?¡tØ1>mL?ªË%ºœ?™'Ž]}?¤|ø\Ê:´?"ÕÉ¿‰ê»?éßì¾ü÷Ú?³µF³Ã'e?µ]®ê‹:?­I"p³Àc?»¢ëhî"?ª0Ar)þ?ïêS"bß/?_& ñ">¢?XÎ4'Äa?T9USr ?RŠ¢6Êb&?NŸuÉ"P?îÏ!ϙÁï?œb–Î
>­?•úu$å՗?'å6ñ›È¥?!PärP˜?Å¤ñX˳?î›åEr.?'âý5¬Q†?œÐÝH] s?Œ&6ܜ3ä?Lš_¿?ƒwò†kþ¥?í£¸4r?˜ƛê´?©¶fŠÌÂÔ?'èÞPWÜ5?˜,i<?‰_jz›rOAGN3FGL J0758.7+3747@fÕø -à@<àu¿Ÿ½ À:—±æ—y.À;û>ß8à¿ÓX¹mR‰@sŽíï@>¥ 5"?ç‡ShTJ¿á'[ËF©¡¿ärÜDäá¿âÅz·pAGNrdg?ï÷|ýñKÌ?Jéð 3̄?A빙ƒà?B9AEiÉw?ABŒÕ?<»ë{«s?ï'èÍ´SY?'nxú)á­?zËÚþ£'?x¼óÅmà"?'9æ˜]ù?Ž¯ïK›Â?ïÊ‰Y8?‰ý~ýS?Œ(]5Hí?€Síx\?p06 ó?}øÜàÂ(S?îóŒ:k"?–'?†g]"?xì^Oþ?sTҌù¦á?›Š1:ÃFý?"íMGqÞ´?ïú¡µƒZ?bhézæѵ?6iÓazñÑ?Zý€ÛDý;?4ˆ~ŠúH?I
å%?ïÕ6wO0¯?s©çia¶?b2P¿ËŒ?Zb@XŠ²?h—7Å	N#?p"0tî
Â?ï'ä÷ÄzÌ?|¬1ä	–?€KžΦ?u=àÏ¥Ó?~NìãԆ?qþ
 I؃?ïÓØ:¥S?pÆIêF'±?T¹bî©ï½?DçÒ+Öä?påŠHA?o[}á¥`AGN3FGL J0758.9+2705@hI#ßm¹A@9òσ³~À9ù"'Ñÿ<À;ÓËwb7-?é]:êGî@†lQöÃ@ —пæýGÜb–ù¿Ùæ×Ê°¿Ü7£8Š¿ê驀'¾ÇAGNbll?ìüb¦-?³zŠŸPžÆ?¶Ê:%Š?²Waóõa•?þ'ô³èó?"틑̤<?áTïú?Èîø0RÙ?×=É÷Á~?Æ­Üž?¸d0mÓdŽ?·ñØÝa$?êüS|
?©ÊxÏ=£ ?ºØWM!y€?¥ÏßVsF?ªœ5ULc?"³›KÁ³?ä̜'ê ??¹krы?ЍüŸo¾Ì?¹]Õû`
P?·c(íÄV?£÷Ñ4õæ?î¢rì û?³4´'OoÀ?¡íƒJ©š¹?ª­[úD?Zuàá? &Õ*4?é¤01²:á?¼( 2:?Ã!ðŠíy?¸"ƒ0ASl?©5:º+?¥¹Ñ/x?íÁÇíXÍ:?}cқ?©¿èEW?šwÇyág?"§"F~È?ƒõ'ÌÝÊ?êµýXìç[?¥Hò/ž-?Â^ŸÙµÐ?£w:4‰h'?™_è¼Ð'?‡XÂáQï*AGN3FGL J0800.9+4401@eø6ŸÏ=À@>‰M߆ã´À9ë̗ó§,À;åáMQ?áÎn"w	¼@
dSÉ&@X?Ý»¿àJÄë	¬Z¿ãžK'gµ¶¿ã•ßû¨­^¿ëǵn6itAGNbll?îùÍñåàð?"ŽÎ.?;'#ôéÜ?"">_
?lU…+ò í?iÖµpE%?íƒÓ9"‹p?¬•,C@/?¦³é¾ØÀ? Ø0{oxc?¡®‡ˆ8?¤a²þh§é?íVtqÓG?ŸÅo}"¿æ?ªe¨à»??˜t¼æ0é/? S5¢P?‰ÇZñ2õ°?ëۂJ{+ù?¦ê"½N¹þ?´
aA¹^?šHù£=´?ª3¾™9i²? iá¼½?ï¾Twâ Û?vv™,Àâ?|N™gXøi?t® "¹$ã?Rªèɑ?PþŸ9äû´?ï+އ¬©Ž?' ¹|­Å?Ž±"œ«?…'"*À<?†VÊ{´X?‰R‰î3'l?îԚ!1†"?Žaœ*­#?™8¯CÛê%?Š
$ ˆÆ?ˆh+æ†ß?sKÈ=aƒ?îÝüßRû?‡Þd«¤~½?š<ðëëŠ?z¾ês²?"æW(
?ý傫'AGN3FGL J0802.0+1005@jw6â—@46'ßk5À:`2g[XìÀ;Ô:0}vM?ÓÈì²44@Œsk\š@*‡?Ïε?äø‡ç2¿×õ)¹Hß¿écí°r#3¿Öåæ<2AGNbll?ïÖñsÂg?p»nŽâ´?b‡ ½½J?cYÖýv
?f‡áØBì?e°'üþº?ï}™ùI?«™«Í£·U?†"gPI®?Žr@Æ
›?'¿<i×?¥Á¶h8Kì?î gã'à‰?—;bµ4ˆP?×¯ébÝ?¸&ì`¸h?žS«iHñ?Šm©'."?ìÙ©EuÙ?«K[Lþ[?¢ÙnP'¦0?¡(-·ƒÚ?¯‹ý]e@?¥t;›t€ª?ïðaRçj?`WyxŽÊo?KùlÌȋ?TÁ†÷AG?Qæ†ÌSPm?R™'~E•?ï·ëUgÕ@?‹gÃy©õ?l:Àô9Ú?rYrŽi7?uìôØØu?…K%½
?ï)ðHŸM…?ƒbù"FV?ŽSØ_Ì?}×¢ž°e?‡r^€ä¢õ?rêÉ?­·?ïhæJ3C?†îôžãÏ?}@î‰j_`?q%oæÃÊ?‡%ö:­›œ?'<ƒGAGN3FGL J0803.3-0339@lƒ@'À‡@,[	 :2+À98'ódKÀ;kՙ$(Ô?ÓNЦ(ѹ@÷êï!¶?ÿðÁ¡J'ö¿à<ÐÀ¼¿á6‹ÐêO¿Úx¯IÑ}¿ã&oI¨¯PAGNbcu?ïøÓv'·?J\ƒ²bá?+×C¬?7?$ 6îáïÿ?Eѯ"ìí?Gødª‡Ì?îåúR8~n?¤¸"Ž''?€}ö^¥™?|škÝèã¸?›º°¹z?¢@'%èÙ?ïa©)üË?²z´™?}â¯q' ?rªÜúLÐÔ?ˆ¤²¶Òã³?yšX"ÂH}?îõcÍb?'Ÿ©ˆaÿH?z[ežð¼…?pŒ_¾e?ªËƒõ¹H?'cu!=ˆ?ïüHÍ?6™‡æ!?$Y=V†àÆ?k»Æ=?3'êEš®É?3™Ù{{S?ï©eT¯I?†gb÷ÿ¨?iâФݗc?aPÔçu?~[íŽ{¿Ò?ƒ`Ü»¹žW?ïµG¿©›?kó™Ë?p©—¯±Î?c>)üë²ó?tÎv'ÒÙÃ?`ˆ½q™¯?ïwRUüûƒ?t.Z¸ˆŸ-?nÃv{I.î?Sÿ‡ÞïÏ?ŠzŒÔˆY¶?r×í`ÄҊAGN3FGL J0804.0-3629@o¡œýç!À-ŸöUÀ9JⴕžÀ;êßÝJÉ?ôUi"í];@>Q%âg¿?ýAŽàØóL¿ãw»3®i?ïõÝà£÷Ê¿Í@X¤u¯s¿âŠ­)楳AGNbcu?鵯÷ÿÖd?À=ñ)oÝU?±\±Æ\?®UR­Kþ?À¡5òL°?ºf§0°?Îe0Ï^U)?ÌÁ5t«ùn?ÍñXED
z?¿kBÆ4h?àê]ºM÷¸?Ë9Xº	g?èÍå?y+?²ÓšÚ"ê?ºt`úìšÈ?¥2¿?Òp(?Š—í‹Íî?­þ"‰†•Ë?äÝ8:1
?À¬I×[éW?ÎQía܂¼?¿ú<i	PX?¼rcpxõ?´¶V:͚ù?í<§,̉'?°k_‡Ø"š?¦ö9ôµ9?£€™as4?¥?S<"R?£Î'ƒÒ?Þ.ÒÉčA?Ҙ¢çS¿M?ÆÏMjcn?»ÿÈðï?Öiž†A?Ìρe£Ñ?ìgo;ˆR†?¤<듘jô?®Õz)î5?œcq»ð`Å?ª³'Do?š7ËÞ+?éH²ƒ²Ÿ?¯ÄºcüoK?ęþÙºF?©ÔßÛfPi?©ão#ïá?ØëÕUÑQMIXED3FGL J0804.4+0418@k/òÿÑÜ×@2/ Z8[À:9Íp`»,À;Î ž9%¿²ÿÖÈû¼6@bÎ
{@‡¾?Á6¿ám, 
樿ìSò²ÿ¿âu-yÆH¿ØŽV,\AGNbcu?ïú ™à"?Aā´"Ö?è`Ì%Œ?÷¸Ö }Í?A›|Öó§—?@'§PèÑ?ïŸóõÒ÷×?‰ÐE络–?p¡	Rq\?o¿4þ£U?düÃGt?"ço$ûæ?îßb¤m°?‰FËÉöh?ƒå·h°BP?v[¤ÔPÈÇ?š ϶ê•é?†NØGe[?ïdÒ©Ÿdù?†'מè?Q¬àáë6¬?T῵þxB?'Jܶézq?…à B
î?ïýŒµ"?KE¯¤â¥?¬sn$¥'?ù¨ÿû­ï?3·Mþ¹¾?Jú†y[Åï?ïÜvñN|?miXûñì?[qÏcʒ?TþoeuF?eýV–­?fŸ/s˪¿?ï~ssº?*j‹³Ø­?xTôöwñ?vt–~ÖÐ?"8¨­w_?v–G+¸?ïæ(¨?_Úμ~?=.Ì^?3ºaˆ9¸?eË*s´(?]wÃ÷_IFAGN3FGL J0805.0-0622@lj	 'RT@*iݾŒ˜)À9Ð%E3æ·À;sŠ÷?g¿¹QQŜ6?@(©€—j?þQìa<°à¿î~»Þ?Š¤›£M¿â½Y4N¼&¿Ÿ+ÍÊ^ï‹AGNbcu?ïïzg,è?UÐ4C\?G·õ=`?A,ì96¯ˆ?U%ìp…ì?P¦É½¬©?ïA¨K¹?›E‰H©í?t'ïé Ú¹?'yÇøÔü?'¦z‹^ð?—]šã¸L?îÖiố?',[Þ?‰…€"ž<K?x:ûð¤ù?˜yò§€K»?X±Õ¢Ó?ï~cqá¼?e¨Í}p?Mÿ'—Vã?Sa _'°Ã?Ž›ïóI?
nXx"?ïúñu*Æ?>'}!(‰?,Óêt\ÿD?%T›/Šð?:
_Ûë†Ü?7ižïFik?ïËÜÇì"<?xÄ'@ó?[ÓÍòç"?UoAkW)n?sNg*'d'?v›Ä"Ï?ï‡vGk4¾?x4{ý8dÊ?y*7}ñûŒ?i¬\$#6ð?Rd*Û?sg£Ò&ƒÅ?ïäGìcý?\P±¾ìsã?3%駕>ª?*õu¨w"ƒ?iSV€ 'r?[`ötì£AGN3FGL J0805.2-0112@kÖ3?Èlì@/—(_ššKÀ9"ÛVÓKÀ;¸Y_æÌ?àBñ¿þæ®@?ìsS4@·ô`d™³¿Ùv'D"E¿è4îV,¿áÄìÿUK¿è²+¸YgAGNfsrq?ïú­³?;Ñ¥?53‰¶†xµ?1UuÈ
S~?5cýËõò?1¨ŒñÝ?ïkKçEZ8?'óOMù?vĞW$ô;?r^pÀˆÎø?‰Ê¶þ÷oÍ?@»t^?ï	Ç'ÇD?‰/÷å5k ?Šj‰*+e?³Ö§9N?'¨Ä]Q9º?€R©§xb?ïZt{øk?ŠÃi%ýMp?j#dýé?aÅ5¤ˆ¨3?'n^óÏqÍ?‰]Æ¿‹?ïýÝÊå°¸?))"?}+?$kD8`´6?$1D,¸7'?pÄý­±?—üò`?ï̟/ۏÞ?{§ÅdwE«?ac¾[œÝ?WÊb­%ë?pþˆðÆ¥?xîŒ5¾ú?ï"¼°0E?zzdÉf?{áUc?t¬íûî}?{X@ 'ú?ku'`\?ïٗ÷,6?i¿öl"ÀË?Z`°P¬?F?˜w¡?i8ÞÄW?f½OdÂÑdAGN3FGL J0805.4+7534@a\j~ùÛ#@>ʙ÷LÀ8Û+6¯ÆÀ;s}°/U¿ú'Cß}Ôl@;ôvH?þ®íÿ!ˆ¼¿ÙÁ‹EmóN¿ß©Æónø¿ÞMdâ­µ¿ÑkFÖºG AGNbll?ïýÒäÇrù?"°¡fû3S?¿¤5±É)?á¼'€[?(ñãDÇ9?™0¹PÉ?ï¦{v»?
º‹&CG?iï@=}|?k––R¼ä@?qùŒ¼ó4?w–X€L|?ïp¸£0Wr?€í1Ãµ?|'ø´"q?w¤­\6½!?…ZÍù??u"™í{gÛ?ïÓü—sWC?t+íBñÜ>ü'øßú™?¨W³wŠ?uå!+mœß?t&LôƋ?ïþ¾Ï‰¼?0žþ"}Ë?
IJ aË`?dÃwÉÖû?j}"+Ï?)æºDßo`?ï䪦©™ä?kV~Ê0?V#FÖOÑ?R÷;¢`?`C¶Ù¹£?fƒ¦¾ÊCn?ï¬XŒø»,?zÂÓe"?tò+ß2|=?w²®Ÿ*t=?t፶Måª?cۙ$¨-?ïøP»¦¬?K-\rÕ>ҝ`">әxᔵc?N™¿«
q?K
ã¹!'¶AGN3FGL J0805.4+6144@caA?ÐÐh@@.é€aº/À9öåvÀ;ãe§ú…m?ôIYÑÇÞ@_!CœŒé@üº€™îS¿ãã•Vœwx¿ëo¼™Ï¿ëÔ5™6j¿ïý2È1æAGNfsrq?ïéšÒ(?i÷S}
ni?Wú¾¯ù€?dn?¿Û½?TϜÎíåQ?Wd[à؝½?þÎãº?Œò|òŠo²?{ï`Wþú?ƒt|ÀL6<?,''Z?'*aŠÙí-?î"Áñ"?˜X7ñÖ>?£€SÀz½?",Yb7{Ä?"¿ Iž?‰>è,«'ñ?ïŒwa'É@?‹P6;_ÙX?}}øžú»ú?€Ÿ*o´Ö?|FVš!D?ƒåÔ,Êy?ïî}ª-n+?l륓?'Þ?WÓ¹YB?c¡ø‡uá?Gý°2Jõ"?Yup¢°ë¯?ïÏ">»žô?tn_'E?fšNøBÕ?`$cUEœä?jCr)Âãì?oÙ²'Vƒ†?îßäN.?"&
ú¢D¤?Ÿ™:¥j*?÷ˆCM5'?U'°P¨*?'$‰6žòO?ïêÌSÍ~ñ?g4½¼?\'…¿wBº?S[÷¨½«Ì?K©¥å6©?aL•x€ýAGN3FGL J0806.6+5933@c³û_ïJ@@J˜?ýFÀ:c/Çmè;À;ïÅôkwGÀ`
+Òí@(õgJ¼è?þ€W([¿ïòÌÒÅÎñ?ïK™™C³^¿ëĎ*XKÏ?Ôb­WD=$AGNbll?ïÝmœÀ'?r´RÐÚêò?cëÝëÒ?m+…@r?]M
°/óº?_o~ù4?ï¸bvå!?€mdfߜ?mɶ!üˆ^?pBÕ$M©ä?téé—KŸ/?wƒ[4ø?îa{O'?•OEæÓ®õ?šÐn#~½?'f—<0؜?˜ý'xõòü?…ð¯ƒzn<?ïõÿ7Ô¿?ZA—$ØP?Æ=ü)‡»?0"k#g&?Rԝÿï^Ô?Yô¦ü¥Ö?ïïµ¢E\?dÆæm*¥n?L<#¾Á\Y?Tƒ³Eí–
?Rv©"[9?[?/'MOÖ?ïå'—²?g©ºÿ½á]?W ð™eV?TE±3ùà?^È»Þy…Æ?a­êâŽ~?ïWŽ(Ē?ˆ]?"	'7?Ž :(¸"?"šÐð*Çj?‰ÉâI§7?xðÙÉíŽ?ïþ͟ýÙ,?0½>©—eôs	ì>±=Ù1²?#j)Ï£Ó?0¸´ä‡LˆAGN3FGL J0807.1-0541@l_?p]@,Ï¡"cÀ8Ât=¿~0À;BñTk'?ðM¥&À‰@2^?Pwè@‹°ÀQ¿:?ɒ˜Y¿àŠÚ‹É™´¿àÙ"v€›¿æB£•4ÉÐAGNbll?ïø_Å&?K|€Åô.ƒ?7r²€Ð?3èßRth?C¿ÈcŠfL?Ešâ1©FC?íŸÆ!•"•?¶ 8š"N-?–ZknS"Ó?–×<P Ä?ªÖh2¡È?²·§wîÖ?î–Ê[¶"?"æ¡Ú\?"½Ü¤C1Q?ˆôgÿ^?˜háÑýÊW?Ýþ¦Î0[?ëiõÀÈí?¨ï(›?¥´À®´Èo?"œ,­b´?¹ÕñŸÑ'a?¦±¦O§~?ïý%‹þ|?,"UT&«{?&XDŽŸ?Ò:]ëô?'%íîkóî?$£á3ú$?ïG7™kÄ?¡Öfpз8?†"DjÁ?‡1}Sý?'óç-ŠÎ?›bÂ9mV?ïP8	0Ö7?‡ß«‰¡£?‡`ïºb?}§wÑéY?"'{ÁV÷?}ì&¶xy›?îQ´¾
A\?\Dý¾?™¡í§ZD?|ð½°5Џ?œ(aNø¬<?Ž§q 5§óAGN3FGL J0807.1+7744@a
¿p@>tþÀdß~À:*‡{‰äÀ<D™`¿é×s¾àóB@Ë,çêŠx@}/`jÎÖ¿è°—YoÕ¿åô©Ä\ß¿æµ´"xít¿â
¢ûd‡6AGNbcu?ïýÃû

?5.¬ày!?#¬á¯ð–[?,SìãE^? hô}nT?$":Í9cä?ï¯ozõß?ÌkÐÆ?n˜Z
>Ž?l¢t%˜I?xü"Óń?|±î¯µŒ­?ïLñnS?"Lû§ôÚÂ?‡mnóq´ö?'‰Œïé?…V5ˆüR?mò)?è?ïÚL熮Ó?lýQ•ºâ?4Χî?3‰äŠ£›r?q˜«@3Äw?loK/²Ùß?ïÿ]Õ͹?v5>j™?—(kz^?€<añÓæ?¬;.9d>ÿÊ(júC?ïâÙih7?eÐŒøI?Y©@7?R܇T1U?`¢×Upۙ?`ÚáÁ[?ï­NJnkÌ?vruè3`x?v'Æ)°(­?u{yÕýJ¶?rÇ»ö©&?\‰æ]îy?ïúіFd$?E~Oåšÿ ??AŽÔ?^Ñ3Nâ?Bõ²™ü³?EöÅRAGN3FGL J0807.9+4946@e'ŒŸ¶M@@9»üÊÀ:$B_öàÀ;ò©1½n?ámyÜK@Q'H—sz@"@ªÀ3¿âœQ:7çÖ¿ãlº4ç	Ü¿ïÿô³à[¿Øùå!ŠòÀAGNfsrq?ïõ"_Ñ?Vg
,o¾å?G*ú—Td?IÞüïŽ?D›ƒ(­Nk?K@yô¯(h?ïZ£É¥¸?›˜J
ÈØ?'2úûŸ£=?ˆÒtZ§?‡$Ãvî¼?"'g¹%9Æ?žâŒZ?"3jcì§?'ë"Ô±%?"P&·»tá?œ^Ø''?.Á‡¿êv?î69©Þ¥?¤¹I(–a?ž©¬ª'g?Ÿ×IŊ¶?š69Ž?—"<®>Ê?ïü
Da-í?BûÓÊ?/3uªjÕV?0ׂ½‹\ø?/øBöÒ?7€9̶L?ïÌ	 Š?{Äïo¤Q¨?g¤C üç?lÕS¤Wæ®?lR±dþ½¤?sÍGð$WÞ?ïO_ðð1p?…¦¤%+?«vHÀ?s^B|¸Ì?Š|ôIç]?'-ì¡ ?ï¶1v´V"?rÛi¡þ?tYF®=R4?mû-ð?pý»?uA5jËûAGN3FGL J0808.2-0751@l¡qÿ÷œ"@*Vì¡~jiÀ7/¬ÎÞÀ:¨Æ¨Æ]G?üˆ—'ÃÊ@«i«kG?þÕ¨%xŠ€¿Ý7I²~¿áå=î¿âuì¶wò¿æX|v{ºêAGNfsrq?ïëb`Ñ?aÙ¼Bê¡ü?PZ®ÇÅË?P;¸Gw?X§-·Žn8?Z(Å-µˆ??Ê_#?2/?k —ÐØ?m7Ãi5t?ƒXçé+ÿÃ?ŒA—Î3g?ì-ÜÓïŏ?§-–D³4â?¨Bü8|¥?š÷I­[?²o›Eû"³?¢í\Ϲ¼$?ïíOh•b?n{ožJ?(ÿ}6?Ñû¼é5?b?ó†ÝÑ?niVžÝÒ4?ïó£4ãY?W¬_óDU¦?IŽœ
 m?L¾]	Vƒã?Gã­0`£?Kjr"Ä?ïÖYúƒz…?xªµ%)?Xñî_©œ?a–°Æò?m-'¡^Ô?t+'mV?ìãfÔl˨?¨þÔ E?¥àÆ[W?œw˜ñ[ªÿ?«éz£ýN4?¡öõʄäz?ïüGm
0?F>¦«T¸?)ÓØaÓ?'Ž;ñ?< Œ/
ôA?E ¹%9'×AGN3FGL J0809.5+4045@fzX`f@?ŠüAÿÀ:-Ÿw),IÀ;Ò½M#Ÿ¿ðÂ^18²#@Ô¾È}1Ú@3
ŸÐÀL¿åŸ"úÚbs¿éz§ä5E¿àF…8ʲý¿ïþ÷b³º"AGNfsrq?ïøžéúØ?Npé~M'?!Y"xz?ý:£?I$…h-¿˜?MƒïI┻?ï–!¶D[`?†áÖÏN2?vUÜ©.?rH'"Ê?~oÎò§^ø?©Ô$ýŠ?ï:Ý;"æY?'Éø'¶ž?ˆ'v£z?tøO 'Ü?ˆÆ/šd7?wæ£:ñ?ïcˆ…Ë¢?‡‰3gWõW?bš''H?d¥ƒ ?';®>ݯu?…Îè\ªÎ?ïüÙd,FÒ?5
–A"Y?¸ —kÁ?|€j‹#?1F»¥rX7?3VÊtÑÉ?ïÛZ£Üàã?k…@DáTó?`¶…`ó"?U¯}ì÷Ýð?cîÖ»L‡?f\wË£·í?ïyªCœ?r¼TUî;?ƒñ!ƒCÿý?jŽç"õ?{—gÉë{?b½éy‹O?ïä¡
g'×?_p¼¼Å~á?:¡Žþ?:G^?=(€?h
ÏeÓn?]¾"KZò—AGN3FGL J0809.5+5342@d' 6m@@wÂ`b@gÀ9ì¿G©ýÀ;èÊõ\8?ÀµÿÅêÓ@ð›äøg°@A)Þ팿ßC߉¤X¿å÷Ù<5ª ¿èßÓr-nù¿Û¥Æ]ÇÜMAGNfsrq?ïütâÙ¡?3(‰EƒÇ)?):Tiؙ†?(K*'åá?/"ñSN…¼?&íÊÅð²?諾›{@?‰ˆu¯Úx²?s;°ÌæI?'aÐX^B+?wfnÙ?}îŸß²¯?ï=‹j(³?ƒ™áÝ&?ƒ,ç2·^è?u;Ì0.ä?p>JvBh?})V#ñÌ_?ï¢h²hiî?'t*š?[CºXÁ¹?Wá³D€¯ˆ?ƒý\zS?ÝFZ?ïþ¢ÖÀQÐ? ÉJ­¦
!?‰¢·S?Õý¸È¯?tXÌ4?¹žSºZ?ïߎàù?jƒì"yŠ?ZØ'Ü@?U'›[
F¼?c»;aùB?dÀ®œì?突œ]U?s êþ?sn²?ùW?hF²L´Ê?wƺ'Ï,N?lTu:þ"l?ïñÊà/øc?]´o.?:9C'?0_Y¹žVÄ?Uâù£·7?[m=ë%AGN3FGL J0809.6+3456@gNà @À@>Y³¿µÀ: ¿ž(uÀ;›]np $?˜³âèdzJ@Ñ$—'?ú´WÀ±5˜¿Á½~r™?ï ú!Ô
àäíç
¿á©²;&ÉAGNbll?ïìG2]d#?fóÛÿ¨b?7¡M­A?@ÄÅ8 ©?`Ĥ(K (?eͽžȂ?îô—¨*M?¡Â~¬b±ì?ÍžjÓ?M•ãkD©?'†NZÈb?›±[ø¼NV?ï
òÇ]L6?fݡߣ?Œ­Z1GøG?ƒáɏST?Õóð…Â*?"Tà"s~?í«&Ód§±?¦:Pií?¦DDdŸA? à^ó'ò?žœËäU¼?™Z³ÎнZ?ï÷Bës<I?S*ð dڍ?*lÓ|ú?.Òó¬|™Ö?LY,HÇ?QªOÈâÖÓ?ï­ÎÒ¶pÀ?ƒv¤€·"Q?sт"¶aœ?s×P'Š8?uG MÎL?|0~Ì?ïw¨Š*9?ƒâO}…(¬?'èöƒxž?OÃ~›Å?~YÎؖH?nÒ)hé'h?ïs¬	³²õ?Ró;z@??'pð÷Y ?t§ñimæ?€¤
{"§?wwÁcªLÚAGN3FGL J0809.8+5218@dÈ,ÿ§ël@@tw_²íþÀ7¦&áìÂÀ:É×5Ü[?ÀåRÓµ@¼ãÊ?SÓ?þ‡ ›+¿á"P$c?H¿Û@°ÛeÒÿ¿ÛÊ¢Ú¤Àƒ¿Ø	ŸÚÌAGNbll?ïü¨">¼?9­äLkΐ?š†o%"p?‹«â_Í
?5TçeÞ$?7鴈"‰?ïÄkê+NÛ?{ÍNñ¸f$?i3©¨júÃ?l	´ËU~º?q06 qé=?ryç;|ǖ?ï2üŽ}Ô?üt"®K£?|[Fx‹Ä?}BÒÞ?'‰œ•ZAU?î+ћçÈ?ïá%}/?mHŸeêJK>ù¦åðÓ?¬Ùi?n§£¦†ƒ?m? 0\ù/?ïþ)®¥€?#¥(Á»Ž£?/ÃL'®?
²Ò'܏_?%™)އe?ëaýó«|?ïæe,Þ
?hæ/JŸç?U¸ªZ¥Ÿ?T‰Vd•rÅ?]}ìƬ?bˆ»~}Ë?ïg,'Nï?ˆþÅG'Fá?zIu3B«?z#—$mtW?‰ è
žr?…~ô­å¢?ïù7Ë?À?EtL«Ð•Æ>íæpc=`>òªìBâ{Å?J¬ÂOK(?EP'TËÚèAGN3FGL J0811.2-7529@rtÿ†]}À5n -1'À8H°?)áÀ;hþÇÜ¿¢Pä®qÁ.@t]%ÊêÊ?ÿ* Htä¿ßÌwgjX¿ß¿Ùwˆ«=¿Üб€7•¿ßæ.<îAGNbll?ïuS\QR?Ž©i¬}2?g÷W8ð½:?o"N†ï?Œ­S!õz?‰¡BmSc¬?í\xÝ Q?ÀG
DkX­?™iã,1?§m±%ªÉ?­ƒ€¥ó=Q?¹!èà 3?ì/]Üæ0²?¤?·Ï/j¶?¡"ìý¥Ð?bq@2jÎ?µÃ	 —Ù‰?¡=4²@?æ™ö²é½?¶SùQÓî?' §z¹ÌÃ??¯îDÂ?Ñ¢"¹=y?¶H~ք?ïŠg\Z?¥'/±¬1?c!â(õ?un½÷i§è?ˆÁð›v"?£>ł7?ï;"DÀÚ?§ê¾ß«?²¾Ž²"?'ëxIíÓ»?l09_›g? B¨"ä˜Ö?î)x›‹‡?™T]¬+ã ?•ñ"`N(À?Š2rj–üÐ?¢o´øe6?"k'÷gŠ?ìOøfê«ì?ž>*Kh?'õÄ&…ÜÁ?r#Ì=#Ú¢?»!"EZ¹E?'Á®"ÍAGN3FGL J0811.3+0146@k–gk*@2Ž³ÀŒLªÀ8NâWxŒÚÀ;6~	ñŠ?æaž39ñÇ@HUñ¤ª@D¿Æ©ó¿Þ‰ÚÈ/|¿ã¬Þâ貿àÚWí¢'¿åÿa"<AGNbll?ïüÙ¯Uºê?-ׅ°ùG?àGN+ZÄ?e'"‡[ð?2úsàâ?*mÆÂÄ¿?ï¡\ú
q?‹¤¨Æ|3?rÀòj•pý?')>–×[?|{vº?Ò!gZ4…?ïf@á>\?¾¥?[´Ø?zûö&֍$?ié
ŒèÖ£?ˆñÌ 'u?z#܀Úh?ï[ƂäT?‹ž="Œ'?\#'¢ ¦™?Y$©ž8?'Äöþ±Ú?‹=S9çA?ïþ—H—¯›?…j	I"ø?6µOIVT?¤`ü_?à=P'_Ö?-¿µ†­?ïØ&ô×]?qyÄàlÙF?\Š:o'V6?T»wç?i"îq{°?mèpÙ:P)?ï¬êÚ)Õ?h½T°˜¦
?pk˜y8ô?Um]sŸ@?yú‡"56?cܲÐy¸ÿ?ïØ!q>Ý?k'7´îzð?MåÏ$b4+?@q·–?p=µsd¸?jeÍÉ:¦AGN3FGL J0812.0+0237@k¢ ¼8*@3=`³žþÀ:þ?5ŸõÀ;'ÕÝÀ¢"^#Í@€èÏa҃?û"éž¿ž;¿äGzr.h¿ásà¸ù"¿Ôê~DdÅ
¿Ã—
f>AGNbll?ïû€]Æ?5ÇU{þ¢?'hK*?!ßö¸ƒƒ?8{¯q*@?1püOšê¡?r;Ëw?›¬3­§æ?h+‹î­y?jÚe'?‡@‹qžå?š¯³ÞՓ?ï*@¶e?‡v~y'?…"ôüÝ.ñ?€d'Iê"l?èç,ÿé?€½5A3´?ïð3@–•{?aC-åÈ>"ª"#?‹>«Pºëҝ?_˜>7	·Ó?aBÑhÂQ?ïý—<òú‰?&÷UD¨†?Ÿ0ô+Ý?ÂbÅÂ:?)<˜	V›R?!¦Ð«t–?ïÜ,=ö…®?wÒB§¢J]?W´ÅÜ?S¡aMp Ð?hPgf`›?uáž]Q(Œ?ï™ÿlԌ?z-WYÇ?w×U±K?t7ì½õn?{(óø‹p¥?l1ìæ5'(?ïýP""d?5Ëñ\\>_3
wö1>n'£í)·Œ?7íõcß?5Ë«R=¼AGN3FGL J0812.9+5555@d> öð@@ºö€$}ŽÀ:3b-À<¦J'R¿²©É{TLB@Œ¥{úø@ã; 2¿â´®<œq¿ä'§n™e¿ââ~=%X¿× N+S=AGNbll?ïæîðtWý?`NïÝ?9Y§wÄä?1yŒ.à?eåÚÎaß-?_dXC1ß?ïiåýê?˜7ú6J;y?{
m[]?‰ÒèIã?"'!Vš?Žì³ïq—'?î¸ÌDŽÙ?Š¢ÞÇ-D?‰œR)Å*ª?sæ€Yº?œDç²ù‰?…PðÔ,?ïf¿/ã?¸ÏˆÌ"?xo&¸ØL}?xñ&€jÇ?™—^g$¸'?ŽÍMÑ?ïõ2à/³ª?eH¯K{Œ:?'ð•¿J#?o"1Ö?Rœ,3ÈÝ?dï-r‰G?ïÕkalÛ?q¦Û½¨²?c–NI†?`^	Â>Ýð?g"Ë»â?i™æ/!?ïv¥·Ø"?u:rº®!?yŠ¶Äüž?\qÉcé6?…'6ɕµ´?quЊՅ?ïÒzÛ,OÙ?k`ÿk·ý?]UQõLê?R1‹^\‹?nÚ{ÛÉb?f¢zÉAGN3FGL J0813.3+6509@bÝß֔Í@@€0`À:Ž'‰ÚßµÀ;Ô¨·CΌ?ϛXŒÍ@
R¢Æ>_@'°?£Y¿ë	G¨'¿Ûw­ÕL¿á:,‡Ù¿èÀ—Ë@ä)AGNbcu?ﯤ6ÅS?x°æ«Zã,?pÖ1[1öè?q³-éA'‹?k£ùE°÷?ià¶añú"?îÒ6°¸'y? ÃÌ;S1?"ŒM*Öy?•v¤‰þD?',ܺ¨p?•à;Ï?î$µ9]—?"	aû$?™ï¹Äƒé^?‹±¥F? ¼ÏŒlJÜ?‰YÇ»n?íE€\ª? !'ªÚWÒ?£w,ñ»õ?"­r—á®g?¨8¯Ïc?•ã"pÓ×Í?ïé à >N?iÜ©6a:S?UìKû{•Þ?`!uInæ?WÑòšÌ}|?\5!TKwF?ïªø®ì??OkÜr¶?u=Ť4¶??kuënjm9?uEãRäî?yØ®
Œ3?ïAÅ<ŠŸ×?ƒ5礆µü?‡Oï|[7?¯k–Ù ?ˆ>Á`üÒË?rZʁdØ?ï(_+'3?€çÐÛcŒA?Û×ýcŠÂ?uۤ슥?"Cø0‰à?tØíÏN'AGN3FGL J0814.1-1012@lütÿ†]}@*m{Ÿ³À8ú"mRÀ;L†ŽúÚ&?Åzm]À>c@K9Ž—@'8`Är¿åÚîÄÕmÁ¿ä˜¢dT¤ƒ¿Û+z	ää¿àDžt¨QAGNbll?ï÷›ýnw¤?Qܞ6Aq™?!*2[Õ?¢V3l?ME~fØKÍ?PÑ8¥¹'Ÿ?ï֞»J!?¡:+"uî?yün]#DD?w›6L|?˜†j!Ï?ž¹©¯?îõ©™…¼\?"‡¬ÃS7œ?ƒª•œ?x肼«?—½J|9²4?Ÿ‰F
?îuÚþú؊?"&Ï4¡–j?bÜדC£ø?`ï¾ÜϚL?§t'"â~$?'§È¯§e?ïüÑÇTà$?7W ¨Øpo?g:Ғ?hõjъ?1—÷z~gž?2qàUµP?ﺛíý?€vwÉlÈd?bí¸·
}?Z«ç	œ?yzն澉?|Ł}Èé?ïŸ^ž¾>?yÛ­N¦?s8û#?oÿܾbHñ?}>2ÌK>¸?qÎ}†P'?-zȯ?qªNûj3ð?Y'Îr?B,Ÿ,t¿°?…zÑ­\D$?qoðþ]µAGN3FGL J0814.5+2943@h£3v@>€'ÍÀ:y¼>§À;ëtZÏY?㪛u(@
O
–<?ÿ¦à©ùc¿îí(ށ¼>?èŽR€«a¿àÜbSS±z¿å÷/"ÃAGNbll?ïÝÖ:gb˜?kžƒU?[<Ìã=¿Ž?]íýTb?d‹_?»·¾?bRÒ¡'K?êqé
9_?À‹pœä?¿"½DC¦É?»&±Ûò(?ª›ô¥ŸZz?®¶ã­>0?îà\¹Ue?Š-«®>?Š¶9"I™?wåÐeÀ?–è"#t(?"Q‰ºX?æƒrM¥OZ?½':$"	?Ñ*:Ú$+â?½!ãïBz?œî´§?˜müÇa4?ïóéä,1Y?]*Ïz9̑?@[JÚ?CèkXä
f?P(4Zº
p?VÑðvÂÎu?3áâf?¢þ"²…7ˆ?™´µä^?™IìVV®?ò©¢›©?–5Rк÷?ïoWà«jÁ?~·F"»EÕ?|,àôM"?lÖ-£n0?†—Ix¾?y·%"³á¤?퍓zVïa?œÌ¤Z~*ò?±g¹-bØ ?šCÖHÀpð?]X•¯?zµH7&wAGN3FGL J0814.7+6428@böW´@@›aßîèÀ8Žõs}¦À;}ЍK­}ÀٔPXÞ@ú­ê^ƒ@_û¿~…—¿â{fôîC¿æüN^v¿à¯±íè@¿ãNŀ'W³AGNbll?ïýsËK9Ý?&×þÇ#/? ye¿ÙÆ?X_íüÞ¯?.óe²v£?$[!£u@~?ïº0ð7á?+IHÝ?lÙVi °?lb:±ep?tŒeö[?v³f-ã;o?ïnŽƒeû‡?|Ð*ÐŽ?w|jÀXlH?fD9>/Ô?ˆž)Ö{è?vªÄ(•?ïæéÑjkY?i˜B••Ã>öF©ÌÚ&'?
ïxö°J?hé¡K'Œ?iƒ‰–Òùç?ïþîwíLt?7[EÙ?©á'äd?kI)!Ú?®¨Q˜†a?ñ‹Íþ=õ?ï埁
?j¢Ïô¯ ?UÊzŠ§7¹?S²Ñ%ÝlP?^ö'Ûîz?dÔAÛù'¼?ï¶éöuµ?gèõÛ
"‡?klÙP
©?Q;'T\?vÔ¼ë»Gè?cï¨3Û7À?ïûõ¿_Pó?A››ÒÔ"û>¸½½HøOë>Á¶ãÝX]Ê?@¤•9ýA?A–†þqƒîAGN3FGL J0816.4-1311@mYb¯È°@(AŸ˜À8cKB±ÂÀ:ßÄ"ïï?èÝÌ.A[ë@ß²ì¦ÜÎ?üméµí¸?hA¿µY‹¿áÔ'€]Ē¿ËyÓ
D¦¿ÛL'æ>ZPAGNbll?ïó@CçáP?T'šr¸©\?1|ì$;?/¢Œ_uP?U q*ŠÑ(?RG¤'°{?î½ùXN©9?¨Ý'¬eZ??¥¨5à¬ê?'{]¿.ñ³?ŸnÝ¢<h?¥§ÎêÎr?î<ZÁ9=?#¦‹5 ö?‰2"W
k?€6¯#"?¥í¯(H´Õ?š(OT7•?ë_lò?§¢s—X?vJìVºªÁ?vc0+?ÁÏøAUñà?¦ú¶‹J?ïúVØÔÂå?@vËĖŽ6?$2R€Û?Nj1,À?A˜Í_¹+?<æ¦'žI?ï™à5¹u?Œ " 
¡ï?kÍÑMI‹?g£tãþ~ã?'"~Yþ C?ˆNB+"E?ïGÃ2Å$7?‰Ç8WB-¸?|Ì'ÑÏAÑ?r͟=o­?©Xáo?†§€²Îç?îT`¿ÞQÚ?‰øÎùÆ× ?z¢‡ÚJ}î?gÄÀ®ÅF?§e£âŸ?‰<ïÈÅïAGN3FGL J0816.5+2049@iMfŸê%@;¦1_ô\^À:™8I©"À;ï"öW
?ÈJ]*lT@
ž‡½N)¯@?è`&0k?¸2Çä–Ô)¿Ûv<lí¿¿Ùì£{^‰è¿éf"6Þ'AGNbll?ï¥W)-?‡!Ó Œ¹?œ¬Š?…oþ«ò*¸?d8Ð:â²?^ ä3Â4x?î›wPæÅ?£.ٌlÃ?—lêÓ·¼^?'²¹D<—v?•#&I
£?ìS¥Äu:?íã'ê†z?£Û|_ÓÎ?¬³ö]²H?¢ù=hø.?–[ éÞ8? -"Š?킦""þ¥?žÉ…eG<? Dy?^BhuÙM?§F€G,:?–Å©ê`
Ì?ïÝ+húÀ?ju쀘€?g)§ß$?dÂ? @ƒ#?WV¥pÂÖÄ?RÀêá Çs?³â½q?‡
"цÝå?|wIl–ea?szõ5Jù?|«Ü¾7­É?'Ç›.u"?îҔ|þ®?•ð,«ã%Ý?›Ž!p‡	q?"œ® ?">¶´•?o0‹ë0'%?ïG‰¹I.¿?2ýĖ'?ŠOãáôù¨?oy@æ~"{?ƒÍ­×Åøh?vÕ¥†Q®AGN3FGL J0816.7-2421@nŠÀ€ù£@ïÝëÙÀ9HÏmýÀ;ohی¿­r†fSJ@Pkþ*é@thŸÑ—¿àf¾ ȳŸ¿ç¾o+ÜÒ©¿è^Ξw銿ÛîÂôdtAGNbcu?ïð_Êÿ?^T‡rÑâ?CµÚkÈb#?DJåØg¯Å?UgM¯‡)?Yÿ®-Å•?í¥7dÄÆ?¸™î‡•\´?|ôhaY2?ƒ+rTõ:€?°Þu™±­½?·WþØÆQÊ?î,@L;÷?–øœ¶f?'²ØpI21?…+ƒ*[7"?£â/Ù{?'í\5?ï7°è¸:?Œù
Ÿ/B©?T°Ù¸«Ë?RS ìK§?—ȇØKçý?ŒÁqgø·?ïúªû²[?AìAW*ö>?0ÂÏBÓW?-]ëbúú?9åX?"ª?<%‹–s??ïr	Î¥¨?™ÚP[í?eÕRß_?fÊÏh¨Ëê?Ž9—·–U?—eU†?ï]Æ|¦™²?€Ð\#Äa¹?¼4# $—?p+U£gz?ˆ°FÎ(i?y±Û<£µ¬?ïÜ*'­ ?eáP24•?9‹tÉ·">?.§£Â«ßõ?pQÿ¯S¼T?eVZëŒ6AGN3FGL J0816.7+5739@cû;@³Nw@@øÍ?¹SsÀ9¦Üx;{À;¡iÀŽ¿çð+‰y@mJ
jKÎ@ç@ó¿ãýæzÕé¿àǵ…Õ¹Ó¿ÙÖ͂»lä¿çj…QãøbAGNbll?ïúœ&ÍÛQ?Aß"#m[?-£l
œ‹ô?1õkÛÿóP?<M†Û?8<ú!'1'?ïrŒXû?'ƒ²&®@?{)ÒPã#ÿ?xzM›Åz?…å³ÚÁ@?Ž´¤,'ü?ïY"Í&äÆ?"C°×ÂTê?{rìý0ý*?mû´8ý²©?‹á–;ë×?€Àº§	F?ï:³}Ñ?Žï›Á­ƒ?b÷qð?$?drÏê‡G…?–^;Nԇ(?
—Õì}?ïýüÜXØ?&VÃ(æˆO?Ö@±š'?}R;–?"G;kÙO>?nË£]H‡?ïÖ²ydoì?nãµ{à;¹?bãžP»ã?Zœ	3y	ò?fiè'?²?gðÓwèT?ï²¢¸ðƒ?mÊllßÚ?oÓe¦û'j?\XÇö…ú?vÄñ ;!P?g†dל¾Ð?ïÖ08ß?nWxÍr?]??ž9Scmœ?<t¦¨?rîF>_Û?m°Þ@§äÛAGN3FGL J0817.8-0935@lúš?Ffí@,¢9 4¾NÀ8ß¾®&˜À;G²3ÄR«?笃›‰ù@ŒO¥¯§x@YIàsÈ¥?§t¹f#Ý¿Þ7Áá
,¿á3צx,ë¿àï›þ< 3AGNbll?ïËØöH=©?r¼&N*ÕÌ?j'Q†¶å?d7‰|;Ÿô?i¤¸®9?hb*št?í+ÊÖtä?ÀIڎNO? _+(Š©5?¦Œd	¼Wº?®.,¡½?·¹}ú"¡±?í÷ÞIy¾?›×Zob8"?œê#¶ȁ?Õ6×Lª?¢
€\ß?'ÐòðA?瘬Cë<O?°e:ÇÆB?³b<
?¤ Êhp6?Çì0¯9Ã?®î`F@õ÷?ïînoõ0n?WªCýÙQ?Sþ`X´?LÄí]h.?NI€	
ªÝ?KþNØCR?îËyrà?®žs'•?äi‹.Ô?›2ƒ-‰‹?–ŒíHIC6?¤	VØR%?ï$IµÍú?‰/m·Û§p?Œ‡;s®è?'¦²™¶C?ŠfW'";'?{%¤q•k?ìèMa1É&?"køqwY?¤…3ÓcŒ9?†ŒrSTqä?¬õöáj?'²ºÒÏEMAGN3FGL J0818.2+4223@fFˆ?Õ%@@³YLVÀ7a{E¼À:Ú;2Ûõ_?öÞÙ|ˆ'´@›:Ö@?ÿŠx»}š¿ß 0öܯˆ¿á~ñ`°+¿á"t˜¼¿¿æëÓ=)V;AGNbll?ïôÙ1ù¼?J¬SƒlÃP??>hõõμ?9F¶¸ÛH§?Lü‰`ù?Cý]Gò*7?ïLíJŠ"?—o¸;õ?"€"'ÿ;?†³²3>Qè?ˆ¨,Õ,4?'€Ž3H§›?ï&ªå­'?³¾KÀù?‡ï‡|T?"Ôh"c?Žeµûõ»K?‡€R%?ìµêµ7|;?§Å™U:¿Ñ?—–7¼KŽ?'ªÅæԊÜ?´keÉË?¦ƒT—]´y?ïûïð?9ü'öç½1?0ÿ—>×¹Ñ?,緖öB‡?6¿ròd?/?%ñ'Aÿ?ï¦êÍ5IÛ?"KàÔÅ­\?ud#Õð?tfcçlG?wzzâJÀŸ?9aåì
,?ïYj2+?(
s?~qǵb*H?uõ1_¨?€ðÁ¥Ò?w9ù`RŸæ?îÄYP©:Ì?¾]ux€?Õðí%x?~-Á¶?—Yÿö{å?‹#ƒ`ôÁÆAGN3FGL J0818.8+2751@h_™÷L@>e;?q/À:30'8'À;ã:ÆG¿ÝS!@	«l'¥^Ÿ@´Þ?ä"¿ãÕgš1Þ¹¿èÓ÷4¬Û¿×ö´·Ø¿ïÿÙÍ|[AGNbll?ïKö¤Ov?š§K®¶(Ÿ?nîÃb¯é?xä"Ë=—ñ?'­m¬˜ß;?˜ßø­äê?ãǟ!ª?Ñ&¥çìÉþ?Ó#(RsY-?ÎSš ™á?µ^ØuÉò?´Üí$àˆ?ë@¸ÆT?©Ð(ðæ¼Ë?­»Œæ0_¿?™"ÂN¬|?·xÔa}?¥¨8\¬˜?è~yÞpì°?¼ú£°Úå?»×£ˆŽb?¶}š–‹÷?ÀFÁõ;?±'cR"Sb?朼?'yz?a>ß?dûÀ«+gb?s½^5?'œÖFg}F?°Ød+?ì
ÓQ–²?½`õcCò?·9'ĉÖ?·žëÍtæ¨? ¯¨÷1?¡þ-LQWÛ?íh)ZÓqh?›®Á'ê¥f?¤Ík‹ÇÒp?—
}N¹?¤¯þɔÌ?"MÉB›ßY?î•xoé?.Þºµóí?ŸÌhøfš?"çÉUÞ~²?ŸÀèÛ#¼C?'{Ì=ֆQAGN3FGL J0820.4+3640@g Á¿½ð'@@pÀOæÈÀ:³Ô®BžÀ;ã·N¶Fy¿ø~&¡l@Ž£?µ¢@Cà{Ö:¿Ü:®%•¿çk	¶©û¿âÑbk/#¿àIq	úÍAGNbll?ïìðzFÆ?[Û03ﱬ?A½º¥Ö??#úé ??]@‰À3H?W¯h"F?溜«€ˆ?…JvåOÈ?qƒ;\˜?qŽò ç?z¶îÂ'›½?€ë;]fÉ?yՀ?%É
0²S?Ï¿`?€¯Âm%ÜÙ?™ëÄþ"ýA?"ΨD,TÈ?ï}yÊ51ª?…Ž'Ó¢l?='Ê~·?@'/.nY?´ÿ0	M«?…N5(g
'?ïú˜õ¯Äÿ?=5-ËA'?'îª/¦"?&·êpoÄÄ??AO{º»3?8yB­YBj?ïßàD›1í?kV
?Hf2?[ë·l?Yp;^ËFv?b)ߓI+—?cV]ϧê3?ïŽe*s"?uÁ²
Ã?zc–5Šž?dÈ-0ßÖ?ƒ4ïÉÏ?ngë~ð?ïìL¾clP?XW®28?ޚðtr?R)z°@¢?c,LÆÎwD?Xô˜À™AGN3FGL J0820.9-1258@mfbŸœèÙ@*SŒÿWc"À:w "@ºÀ;·+rt'¢¿òzí¿`¨Œ@€â¦Rå€@,Ó P—ó¿êâ=‹Ä¿ây'vg¿ÜõF""ð¦¿æh¾òæß?AGNbll?ï¿<™ì?ò‰|ÅhI?c0ƒ¿^m}?i®å¢sÂ?vٟ½Ðӓ?{=´3^?îǘí(?®+âoÁñâ?xfñW™å‡?ƒ8ìúw|z? y",³ƒ?­kм?î'^æë1?™îíÌXƒ?"ŠgÔV'?"ç«×ò‹?£Åá®Fª?'âõŠ½%?ïL•Š@`B?"w¢ÊZ?HŸ@ke?EÉ÷<P£?•¨T·+>·?ƒê""%?ïô[¶Mô?\öù˜ž!2?6ø—
7ä?5Q!è
#Ê?QŠm ý%?Y­6j±_ð?ï´}¦|‰œ?ƒªßtì§c?b
º'ٍÐ?bæÆ^ Ú/?|ºO‹rSH?€]Xy8?ïbY½qÌ1?}ú[¨S»?~›w@Œ?h±"¾3È?ˆÕS½_?wžoֵۜ?ïÙÊÏÐ	?^zÁ`^ÄÄ?-ºÊm^?"~ýLe"?r,Áª[ë?]¯â‹ÆâCAGN3FGL J0822.6-4250e@pE•:À
5ðŸºÅäÀ7A9†3‹À:H{$cŒ—?ñÏoÏpÁ@}3¤GG'@iº?V'¿ÉŽ;l'¥¿ã3݆Xt¿ßŠRiY_î¿âýŠoZ*ïOTHERSNR?×ðu¦\?¼«Ñï:NÊ?¼ájÈ?ºKŠ=Â>?ç}â5S°?ƺ´hÊ;D?ÔBNKuä?Ñâ2+ߟ?̲JBq?ÁѬ#ß%?ÝdrH¥hã?Ìi"9?Êh¤Y;/¬?±•S% ]ß?¼•§"ú•ª?¦5µÓèÉ"?åÓ!ö¨q?´Iq'êX?ÄÒ3Ð"R÷?¯}¼Ik»?½S†Wûó	?¬ð±ö‹ Ö?ç!@n|'?µFÙáMÜY?ÆŊý[?Â'vsq3@?ÀªapêQ?Á]zçIG>?æQ3þy?Ì>¨*ð³K?à8å6"?Ô
ÄÉH3?ÈM&›Â‹"?ÂiKÀj5J?Óg¢Føs*?Ê×°š¬?ÓÿÇ´<»¦?¶EÜÿîå?¿GLÖÙ|D?§ú`G­,?â2‹r¥?¶rÚ&_aÑ?Ñ
"ƒÉy?³"òÈ:ë?Àª6Õ"ö?£F…in«?ãP(;Tâ'?µƒÁïbÉ°MIXED3FGL J0822.9+4041@fŒ8¾øγ@A`	UÀ9Ê";ÝÀ;¯ÌÐþŠµ¿ß®Õ'[°ø@©F>RÌ@éà‰¿ä—ìëÑì¿å¾Ó¨'·¬¿êîCe'¿ÑÌÎû%OÆAGNfsrq?ïüèK¶ëB?/í{Ã̀ù?"ë¡`d?F+75?..qRý?&á'ôeJc?ï¸9ß½H?Dñ—I—ª?l*|>¶?k½¯‰V?uÎ3€ë4Ý?{Qí±gwN?ïXMùÚC?|¶ŸÀ£ii?~X­ÈPs?jeB+ ü?ŠÀDà!ä?u´¾ÜÉÂö?ï³çi—YŠ?yô2«œ¦?='zÀr
?CUr—9~?'ÄcŸÊ?y'hGe
?ïþoj­.2?!Œ¼H7K?ˆ­‹'??åؙ=*?Š2D±?ˆáCY@?ïã¾ÝºŸ'?eq=·Ê÷Õ?WB'xw…Õ?T3ý¿#8?`ŸÙSŠÂï?^ar­æ2?ï­ôŒ{ÆA?lë]¢m¶»?qR–S'¤?ZW¸â*ž?w³#¾)%¨?d¿ÁòŒN?ïó½E+"j?Tˆ9MÀ."?7Ðyæ?p·§?W$2PŽð?Tû˜,ÖAGN3FGL J0824.1+2434@hàéߗª¬@>Šô PmÀ9Í]®1À;¬'Ä"Bh¿®U;¾˜Û@I¯K‡"@$e –"—¿änǬZ/¿ç	®éî¿å—÷9v²ÿ¿å°¾Õ˜AGNfsrq?ï÷êdY¾/?F³]P8'ñ?3SGqšŒ?4õ2á¬"?F¬Ê—¨Üj?BT±^ÄO½?ï'Ï\ìaŠ?‰vóû…‰ý?v×÷úY?r›g'KÆf?ÀZTˆŽ?…X!:s?ïZ
ÅG?f~[%?|2LkY
?lèóÜ̘K?‹c™ŒÁ_?|.˜³,u#?îð¹¹Ó(?ûÒ|lÀ¦?v\¨*ã¤Ç?i]‡êJ".?œQžµ
®ó?Œ€p—†ˆµ?ïü…hÈ?2Ë¢–?$ïˆ ¢à?$ù°;aÌï?1\ü'zi?*劌ÖÝc?ïÙ@œb?mðÒîVZ?aQcI­?X·ÐoNVw?en	EF,?fÙÊ
_?ï³
œÎÐ?rénýù?o¸R®V÷ª?b«¢†ê¡?vRã\J?oiò?ïÅiµ6"M?l@wn<?[=ìë=_¹?C5ÄÂúß4?v{ª'&Ñ£?jg—$߇^AGN3FGL J0824.9+5551@d?n «†@A'Ÿ¸—ŒÀ98cϳ1À;ÑF2ê8?Á ¸è®@¢é¹íw@ÙÃߓMû¿ã\<´š¿ê^+œ;¿ä²67ìÍÁ¿é—ÐAGNfsrq?ïûþט`?R<TZøÚ?Vëê·Rï?_ßèÕî?8sÍÞ-Uf?RXïgÑÕ?ﳟ/'?ˆÃs¯:šÐ?põZèµ\Ø?ß"$œc?u†ÕD.À?|rQ·pÚµ?ï3J҃'i?†PU½R¯›?w›F/ÍÃ?n H¶,kQ?'¸¾ÝQÓ}?…sx Û¿?ïÛ÷œÀQ?sØ	¯"Í>?@
&ù¥??cŒrHgJ?p|?Bz¨?sf-R;ë¢?ïÊÝ8LD?²ìԀՐ?nÈÐîÚ? AŽÀW?z¨«Ÿz?²r<]~`?ïãØDO:P?hg÷鎭
?XŒ‰LWº?TS'f¹Õ?_Âî™$¥Ž?bÿÊړ?N4§Ž?94Rb»q?tößêéœ×?fpk`=ÝÒ?ƒcüsjp5?€V¨À4?ïúÇômG#?IJ0µÎ˜?!U
˜"6?˜qJ"Ø?@ŠèaV¹?H-ÏÚÙNXAGN3FGL J0824.9+3916@fį_Ô{î@AU_­åÀ9Ć4b\À;Õ½5?âm¸¼Êv@jŠ'T@>`
ø¿èžŠçq‹¿ÝZ"e'¿è(ð@¼«¿ïÿà­Õ:ÚAGNfsrq?ï²Iù?Š
'rËÿ'?M—sµÀ}?ˆà?dQµÁ?Q_'Ø_Î?Y8ýñ‰¥?ìæ
??²Ÿ†ZD?­'g¡#ü‰?ªÏB¹?¤/\*–?¥«Y!ò?ëãR¹qŒp?©KôÉ`É©?¹æù–%é?¨…öøºÿ?›ùÂtc¤?'XížÛ?ëmŠ®*†x?®î#ƚò?»Ñ¦™dóþ?¬AâÏÖ]?¡"ç?—˜ÐËþÔX?ïÀ¼#/@?',j'£;é?|q¥6îB*?V¨›N¬_?I€šàf¶?P׋1îÚÕ?î틷êΧ?"¶na"`?•}!"Î~~?§}÷™Ø?‰¢ÎáõV?‡ƒE3)¼×?ì â™p\'?¥ßTߌ_M?µÒ×a|üé?¤N â]4?"˜OJH¬?‰Äwg
hH?îõUEñj«?‹ÄWWý/?™¥Ü"&ù?…uk¸Pb?~½ìÖÆÖ?|Zj鲨‹AGN3FGL J0825.4-0213@lFÔà—"ì@3®Û@-¹À:S¤A"HGÀ;Ïçû&|l¿¸Åb$Lm@	2Á濽@5œŸ]}ß¿ç\ÄfZ6¿ä7;‰ªˆ¿æpÇNaÖ¿æƉ"ßgÑAGNbcu?6U•? AQoc"?T²ßlê?\JŒiÒûê?‹;Vh"›d? (¶¥À"Å?ìU7ûw´?ÂzP.§Äf?¯iÔñÞ?³€H¿ÖR?«B«…±-«?·S"ºdj?í€re<´?—×&¬÷"?ä؁?Š%ú"xǨ?©0gD'?' FIbü?çIýÙt1?µ¯¹ÕDÇ?¿žqðˆ=Ò?±U•.ú	3?ÃÏ£RT?®tãt¡«?ïÍØ6ž‰?ŽÆm.£ù¼?:-ZºzÄî?EŒô‹Z«î?w×> ê3Ð?ŽÇ"?à$?ï%aµ|¤?§ïWp7?Þc‹P?šÂÑ\´$?‰¥	<ÔA—?›ÿÂýÇê°?îês '¤?ŒìBiú'?°š7†ü?"á?lôÂW?'ÔONÒ?æ·o"|?힭»ÿ0?˜œžñB.?¢J×$·.?Ž¸º=²)?£ÊW1Ø#Ê?Ø×@DóãAGN3FGL J0825.8-3217@o"Àh¡@
i¿ÿ´ÖŒÀ9d8Ž¼ÇÀ;Z|¼A%¿ýÿÈØK†@{ âù‰ï@ê®YÒY¿çq¼*	¶/¿äó®é¿ä§Úb{d¿êk…xêAGNbcu?ïãíÚäh?gúȀ[]à?_ÜTÊʤ?_Т?ZbHJ¢µª?Y8šU?3?ëˬºe1?Ð5'g,E?Óg}Þ?ŽT(:¥Q?¿¥c¸r]ý?Ïn²5—¼?ípN?0Ë? ëWÝy§¾?¥m‹ëþc?˜ÀT`Á?£à®€+j"?'Âέ]×Þ?ïìN~¬ó?e'desÓ>ò½"k'ü?ì
˳ø?cŒœf4?ej0¥ƒ@?ïñ¸Ý̄?Xº¤ˆ¸YN?Rèbȹ ?RÃ^G‰°†?CLa$‹l?B	«1ƒ^t?í¯…[Ê??Ê%Ô@ðœF?|:°;¯Ì?"ŽoÃ'·?°Ã±uLk?È<*Õ¸ü?îóàfK}F?Žýp'_#×?'2xj²û?…ò
¶èX?Q{.ÜD?£ßì?ïü(L¥J'?<p*þ&i˜>Â$UN»÷>Ôj*ŽØR>?>™p€–A?<bæuыAGN3FGL J0825.9-2230@n~à°¯`@!Ùäúœ>À7ŸA¥ÃtÀ:Èï'j¨?çÏ™à@4%죬Ã@cÀCÒh¿Û‡y§Çëοâè$Zìú¿ÞíñN{'¿Ý>"[U!AGNbll?ïìY1A
?bY²pLŸ?8ç¯ýë{?8
å+Þÿ´?`‰Ø¡æEú?`@œ£r_?îL-H@><?²Ãibw?"ûlÜ_-?Žâ獺µ•?¥þK"|Òp?°Ki#É̓?íŒxGJ¨?¤r˜4	Š?!a;¾£è?‡?jê}¹t?¯p#:®ù?¡ÅZàÈÃ?ìùFí-?¦nîÇ´º%?x©G"Å›"?s¿†*Œ ?½•¡M©<`?¦¦>ë
¯µ?ïúˆi<üØ?>ðÓgz{7?"ë,MÙ¯6?:Ãpí?A#²7ÎG?;õ_Å?ïhÑPÑ:?–\†Ô7S?r›
}Ÿw†?{³Ñ­¢?Œ~&œX#?'à—òßâÒ?ïºD‰ò³?'ð-¯;L?€€þû?yµa×!˜¹?—šÖ3 ?'àRb8ß?î¨ê'Z‹?‹íêf¬*˜?s.u]øø0?`6¹©0r?£ˆ.Ä*ë?‹ßa:\¼&AGN3FGL J0826.0+0307@k¨ø -à@6mÀÊ`À9Ýa…V¶À;¬½D¦"¿ìïAïíö@ 2)gW@<Çÿ]˜·¿äàÿÆì…q¿áT'8§;n¿×ô'ª,¿ã)ç/#¯AGNbll?ïû÷µâ-:?2•?!]]yá?lãÜ}?7º¢Y#-Š?-ïòDE-?ï£þby¥f?‹¥Ê{úýV?s	‰X¾9
?'Yò*?z÷EO¢ ?'^%ÂÕ?×ܶ?qÄ,–ì("?q§:Lgš?Z§6ðk?€'Û²4Ç?m'ÚÆ$Þý?ï—Ù/º?wrè"Wè?7ݶO;û?6±t<¡ö§?‰|Q5?wvãÔÁ?ïýÀ)€h?$5ö}›L,?2ùó)Þo?
"ˆ®1¸?(åÿ³Aƒ? l5Ý`6_?ïÝÞôRÞÛ?jÙt`*?[ ÐyèiÚ?Sæ]"`C?dP£¡§O{?ei³MKïŒ?ïÅȶœL?iÈU`'h?fŒÅ»('?M'ôÐ`"R?qÕBν?góžë¹‡+?ïëA`-ÎV?Rf<SO(Î?!oÈö•?C°AJ?c­ˆ¨GiÆ?R`AGN3FGL J0827.2-0711@lޛ6†¥@1Š	cr–À9ë:^ ŸGÀ;²ÔG'‡¿	äÐçž@
j°ëoÐ@‰žŸgäÁ¿ÞÔl´Z¿è~{å˜d¿ÎƒÉÈò‰¿ÙD÷}$™AGNbcu?ï§Ã'Be´?'è6"kª?Kt6ýYy?ECGËl4½?"WØ0éŽó?'dl«ïÆn?ï^®)Q:¹?–¢¤Ã÷Í?xpœpÉ¡¶?vÈÇn8ù¹?Œ'eæ?"'hš`Mz?îeWükK?•O>ªÖE?eà%ß?zé<ÞÇ?¢a¡£ÌÜ?'Nþþ"½c?î†B÷mז?"´Apç¦?d¹^†J=Û?iWpH¢90?¦P:žð@?"0/·l'#?ïÈ~.·¬?­·X)x†?@ä.ћ?g,A˜Kõ?y¤f ¡·R?­oÞê«a?ïÍ]NmSô?yU'4ôŸ?aÝz1Ýè:?Z­Ü`Ú[?pb›«—ì?tš!«Øª¶?ïb¬˜­i
?zÓÒ¸¼¥?|ê|l)w\?g,¾š	B?ˆß›¥p9?ußcÂ?ï­"Î%4?nvw}Õ`Í?[²ƒ‰°˜?K›çÊÚW?C
\ x?k_Šß¬uWAGN3FGL J0828.5+5217@dʽQï·@Aã(CìÀ:ÊÐþŠ´úÀ<!‰X¿ºáӞf÷ @g¤Ôá@'¿ãZX¿ëê)1°.å¿Ö6¯¿ÔOÙìðڿ당Šá×AGNfsrq?î|Œ³W/è?®ˆ9ßož?§eÛ«P¿û?­}­>Œå?Z+#õF¡L?b#v²ýÙ`?íNñRF?²†­?«i ˆ"AI?©œ«çŒÝ?ŸO"¬Ž­œ?¡p•0¬¯Ç?êÄoì:ë?°)lӃna?¾ >4ª<æ?¯	ӌ†@?¦}¬"x;‰?"§žˆúaœ?í»4ÌöŒ?£~ÄÌ»>Œ?£+Ùb1xs?ž^S±þ¡M?¡ ÙàκÍ?'w¸@ÛÁ?ïjl+CÈ?"=kf›"?'2óׯ}&?"€m§É?X¯ê¯±ìö?ZžóM"ž??ïi›÷Óó?"2Ú«">?…T÷(?Ž@{bz]9?€jaßú?6?0˜À!Œ?ìܚe©í?¥//†jÅ?³c2O¬'O?£kòd³t;?–ßöVPG*?ˆ=A°Í³j?ïss)9׊?{Þ¤ÙU¦?†cBªöä?s؛8ˆc8?yçKëK?næe>AGN3FGL J0828.8-2420@n¼WÀ±5˜@ Õ¶`#× À:6ÄíÛ:NÀ;±Ø{V¸¿æP˜#Lá/@
Ū‰€ò¯?ÿþ½?'‡¿ÒLS'ÿ¿é×:$ȿȏcüï2¿ãˆŒ£^aAGNbcu?ﻃ¢?¼f#ëW?;%*œÁ‹?:Þ;Û
b2?€Eî6×êü?HO[
º?î
÷¾¬½R?µ2Èkáqí?€fåùún?'9|;M~?«üØßþÎ?³îÂ0I·?î ƒ<ØDò?˜£Áe»p¯?Ž_±žü?{©Ñ'?¦_ßÎ,)q?•™Ö{¶?îý+2nùC?Ä'ë4ž?E>†Ä(—Â?EÊ6qåv@?Ÿ°¥xÑ®?wqÍ«M?ïð¹ôáq}?]¸Â=wÍ?*…óŒ?'˜xU¡X?[I%%ì­?\×»xq˜?ïμ¢C?"If#j†?e"}Çæ½?cîåêÍ?‡xë7ì·k?'º¥ß¡[r?ïD˜BMú¬?ƒ	4 õV?'•EfÜl?wԝ§¡i?ŒXZ!C""?ygùÅpu?ïɛ€Š»?g…ñ;'L?;Ÿ¹ ªI½?-ëCe+Â?yxD&K÷V?fÖ¥¡¹E€AGN3FGL J0829.3+0901@jý؈v\@9ÓÉ¿Ò‡À:¨L…ЗÀ;à\KZqf?Þv~;U}@c‡'ÛåD?ÿ(ÜP'`¿ïÿÕYu?ïýv8t^¿àò±C÷.¿Ô÷P0;~~AGNfsrq?ïïHW‡¦R?Tƒc4HU0?HžG­]{?CrbsÖ?U Dt O9?Pn@ø
?îŒùF8¯°?¬¬ÊAåÐ?™Iªèì,? ¤¬½Ð¿ý?•-3¸ëÏ?£0Þ¯£FA?îäbF"…?†ž±ïAdü?ŠÿXTÊÁ?}ˆ"9—ý?•ÿGÆ?}'ø‰=ÔÀ?êȀ«ûµ²?¹lcö1•?Á,qšnx?¸»2Ý­,º?žÆ†ëÐ?œÔ@ê"?ïø]q +Y?B¯õÜ|¡s?4¶Ë@Bä?0n¸c7@Ú?D.ÔtŠŸÊ?;nðâ‰Ó?ÂBÍ?'ûq©½3?ypÎüªD?õ»5z%*?}(.»/P?Œ "ãö?ïoMFɁØ?y8EÂÂ1?~ÜðìqÄÈ?rÒhRà?"¾5Û.9y?lŕ·"Õ?î͊ÍMü?'ÕØ£Àp?ž•¿
A?­Û‡P?~㝶!"?wË9'íÛAGN3FGL J0829.6-1137@mf[ ¥&–@/\7 þ}IÀ:SÐ-hïÀ;¿ŸàÛwŠ¿õb ¼8*@AåÀ8À?þ;Úß_ ¢¿Ê±¡NU	¿ìF»,Þ§¸?Ñ~°ŸšŽ¿Ôr¨©ïAGNbcu?ïû@UZ¥h?? àÚ'ì?ˆð¬Ú?"|+¦g?@›˜Ï—\?=.f	g9?ïüR݃º?"'´KlR?kýAk#ŸJ?kø¤î>½ý?‰šß¿Ã¥?"™z¼"?ï{"?‰°+èw^?€ù¾£?t'"xª,*?"0¡êhAœ?…˜ÃŒ°r¼?ïײ›$??s2\6uR>äžËI¸>õS‰ÓôÃÖ?t¨ž‹§?s‰Êm›¿²?ïýªM¤2?*Y»™Ž°´?UrâNÉÕ?S©¼êIñ?-ÅÅ̓I?(|U•x—ª?ïÜlŸædÎ?rñ®MA½?V6»czò?UüÌÚË?hxˆÙøk?n"Çd×ê¾?ï‰MÕ…?{˜õHÌ?tÉëpüó?lߚt'?ƒGÈ¿jšC?w/ðü±ä?ïú!ú#¿?@囷,Ë(>ØKCÕÀ>Ü«T3²Ä›?GKp'l¨e?@͛¹åUŽAGN3FGL J0830.3-5855@q%ˆ¿Â"OÀ&ã
F:À9Z¾ÝöÀ¼À;†aQS°?è3ˆ2˜ü@=òFƒòé@Ý»à~í¿è˜p&Œ9¿è¬-ÎFl¿äÌ~?Ã\¿ïÿ¯í1àçAGNbcu?ïÊ7û…?}šú=°|?ct(ýoË?iͯ§ICå?q*cÕ·1þ?t	§$¡Â?é€õ¢ž?Åèys?µ…¡bba#?®F¶a•5 ?ÀèéKf8w?¼g0Õy³d?î3ªÃG?–o.»?Ÿ@òª¤n?Œ­Á·4Ë?šN؍ò²À?Š3<ø–Æ?éŽ]í?­–ÁÓ™Ý?¸ 7þ=?£urô¸?¿+U`I?¥²¶Åà?ïÇëGûÛó?ƒØü@çօ?hqÖ×Æ?rj§è?p#å
¥?xÖ,Ò??ìÑat97Ú?²쫳y?¤¦èý#Ÿ?›oԓ—(?®Bÿ»Ù×Å?ª¸]qMµ?ï'nr¾'\?'Í¿'?"Àáµ{È?z³Úa"°?…ázÍV?sA×¹Vw­?í_n£ˆ?'[lg{G?¦"p (³?†(€¢îÚ? z{vaéÒ?‰Š¦ `~¸AGN3FGL J0830.7+2408@iòà\̊@?Ô· "À8¯â*ðoÀ;'çf¬"?î,Û`–÷1@è]…TÖ@í?³õ¿å@É-}^¿é6ÀNí¿çr
²©`¿ìm«ÞöAGNFSRQ?ïóø1¡Úþ?LŁVñùì?P•j"Ú&V?HãçÃc?=èǹªÄ?6[淂ÙQ?ï•Rs"?šÝ)ÜàO½?ŒMÜIð?†¸
ü¦?á帬?•År'Ÿ23?îü;Ñ׎?ˆ4Õȕ1?'ÈæWE2Ð?*fNGE?‹_>ÔÑþæ?z³à•H%…?íÈñÅ÷èÒ?¢¤¸1c? îúD
c?ß}{'?£_ô¤…š"? aûËýj?ï÷U"ýšÂ?Da?w)2â?Kòû§ý=?Boy¾ŠÈq?*Ú͝Ыº?!
nÎÖƂ?ï Ñže'Ä?1¥ïÍ?w|ÜiãÍ?pm¼°ò¿?x³ñ:?zq¬Gª?ï9
Eôè?'›C—bî?ŽǗõÏU?~‰Þ"YF?'ßâ
†½R?qñ¦C"8?ïk¨ŸñÍb?ƒÅò£+)Ù?…gö"s$?oä?]|,€L{?€\,%uÎðAGN3FGL J0831.9+0430@k–Š r~@8^'ŸªTÓÀ8&–5À;9¯4^¬?ö wÔÍÍ(@*íEé]@°Ì`Á5ë¿Ú~Oû"´õ¿å
‡òÓ¿ä2z ë¿çC^ˬ*/AGNbll?ïúsmNѹ?:þ¹§£å?3Y©Nš?0ÁäIÛ¢?9\=a@'?0é^7»?ï¤	¯"º7?‹X;ýÈri?rw«ÅW˜Ü?'LsÈ
Á?{ƒ|¦‹›Ý?XAŸRX?ïHçiÓz³?ˆÅ¨©'Š?…nïΎֹ?¦]Çdß?ˆW5®Ô‰?w0g—º?ïœÊLّE?‰P¥V£Š?\âÚô	?fs´ º?…1cãPÞ?‡ýLtâOø?ïü°'û?>ÕLIJѱ?/í
{k?3b˜eŽèw?%	ÒxWA!?+¾ìÍ0?ïÛ³	'4Î?lå÷_K®?_ÞóÐý ?XH•±\ÍÄ?d]|Z3;?g/ßý½@Ï?ï''ÚÁ5?|épþnÕ?~0ÚæÝn?lÅw¥ŸR"?€g-ʊE?w2M%;ê?ïéäùGØ?dS[¢ã!Q?Pm.…
@f?JR"Ÿt'?[ÈÞ³+Ÿl?a¹AkaxBAGN3FGL J0832.6+4914@eC[ÿW~@B6| À:¥kÏ[óFÀ<>ô1•¤¿ÑHe²¿ãä@
'žÜsß@è? ©Ù-¿ºä¸·þÝ¿é+'Ÿëñ¿àöäð§j¿çJ+í;#ºAGNbll?ïµda£2?ƒé_?dñ‡Á|?l¹©¬þ¥‰?{LJÀrT?fõÛw?ïjž£ˆt?'H2Vò?àósHWÎ?ƒ¦n³Î¹`?ƒwc«Jló?ˆ¸ÆRË?íð˜ùƒ¦?"æ8—y˜?˜u¯'Íå?†ûh©}5?¤»˜Óé$0?0µ|žr?îÞ6$V?"cp9ª?^üig?u)B\›Ô?œa}]É\?'|nÂSÃ?ïï^º z^?`L!bƉÀ?CÐ?¾žñ#?CõT9†W?WZj 'úð?Yþæ¸KÚv?ïΉUSÄx?r›ÿSHƒ¨?fŽþÚT}?`ŠuýA»Š?jç¬(¿Ë2?oãã¢xÒ?ï:-Ǩ:?€ö;B
»j?†w¯Âƒ{S?x–Œ¢Nï³?‹"½Ô^?tZÕ¯æŠ?ïǔu‡/y?nZÀcJN?cö
®)v®?OÐXóíó?r:¾DWH•?jª¡,§ýAGN3FGL J0834.1+4223@fSëßL+R@B'±ÀoÀ9f:¢"=_À;Ȍ{£åM¿ôž6ìü=@<¦Ú'Q@ƒÀ`óJ¿å«cÛi8¿ç©Á‰Å©¿ÝTPф~¿é£Ü^nAGNfsrq?ï—8Rÿ?ŽÃÌæ%¢ø?v·ƒÞb?{aK¸ÒÒE?}¬ÕôYQØ?Š#lƒÆOƒ?ïy®sµG?'|-5í·?}8s`‹5G?'5+d>?'ø)`»E€?‡‡ë«¼H?îj½Xï
?"O4år²?'ðÅÐYIG?"J¨•	? [LJ*»œ?'
(Á?ïs¸xF?"±ÕЁ3?bÐðOã2	?hbé&È2^?™Â"yI6
?"–Öû«¯?ïꠍ(Çõ?gў<Djš?Wwn*ýp?WÓ …?SGÚ¥ù‡j?`îÙsŐÁ?ïÓàÒ¾(o?uz½ûi"{?cšÏ?f0)æÌ?i´Y±?k1]éÏâ?ïd·üw¢?m¨>•ïm?át©"q?u†ƒÚÄ?"ðŒ?tý1?w?u(Ӌ?ïÛ½}EóL?gÁÀm©?4*4J0˘?9ý6G÷ÒÀ?pޞ/"Pç?f"»Í‰RÕAGN3FGL J0834.7+4403@f^Ñ·@BH{Àj¾»À:l{¯£ÇÀ<Ä3¡<À¨ˆ‹ªB´@%š_'6Ï@½:¿™ˆ}¿ê#"±*ãa¿Ïh
Ô"	H¿ä&\tŽáô¿â7ÁGˆÁAGNbll?ïûXS±¶z?<¼(n?4«øg墖?7sÑ}"TÅ?0'i0²…½?%´ÜÕg?ï¹Y]"&?ƒQ
‹«Žž?l•V™Ü?k—% ¡i?uPµ.àe?~Jˆ`H"?ïªHD?‹é¸teä?yi}'"?"a`Æ&?Ž
Xï;?~j;V.?ïëfÓ2º?_éù(®s"?a/00Æ×? ŽÏ¤`!Ÿ?cþ#?uåÎ?__ñÙÖÞd?ïý]Gü}?0TL}a?)kOV«u-?-¨lhŸô:? À.RtÌf?_ZžU?ïç<¤@?dn/FU?V.?ßæq?R':æ	ÿ?[Xw€äÌ?[¶GB}·?™Û͊?x‡Z3èy?{B¢Ù]¥µ?uKÛð´?yù#n+?aZü>Ä$Ì?ïü­0‹tN?;8e-kÀ0>ÖêC'2>î¬ïþŽ?::ÑÌëzE?;"Rÿ$ÉAGN3FGL J0835.3-4510@pxß¿ƒ8.ÀLV ž9À2ˆ©ÀXJDÀ8Çå"S·@衦ˆ›@ø9'rÞÅ?ôž£¼ˆ1¿Ð†bbÔ>¿àÝskâ¿å>¢ÔšS¿ì̋Ç0PSRPSR?0Zål"rz?CØšÁÎ
?Ü^zG!…>?י:4%³?áη€ã¢?ט£Ñg!ˆ?1säîÐ?jà;½Ó?ì"48ÿÙ?¿ñ~õ?»TÏá»W–?¿ó–Б}k?p
«Å¸&?s̎*Óý¾?ç䠗Jðû?¶ÿëFÛ=?Ïí%MӃ±?¶U[ÓÅ¢>'UxÑø¬
>¯OR5¢zé?ïSÁÚ;±m?¤2¢žãËæ?•‡²\ K×?¤2 ƒq"Ó>÷ÞiYçq?t	c?à©ã¨],?ØCRìr?Ê?Þ«Ü4ÒMH?ØC;õµµj?4euÜcƒ?bu‰lO?ëÏ夛;–?¸…ÇMJÐ?À¶6±¥À?¸}¼•lR?~Ž¨Ù	gy?‡t
õ™Ç?è
GÓÿ?´©™"ØC?Îã)˜Þ;h?´t6£·>'¶§à	!>©á:n¥Þ­?÷šU×?¨I™6~^ƒ?¦e'«xeÙ?¨I˜/¤AðMIXED3FGL J0835.4+0930@ko?Rü&@;fi¿·:"À:WozânÀ;Ô$n:¿Â"+l=@³ieIZè@OÉ Gˆ«¿ä'Õ""¿êV_T?·¿Ñ©Îée<x¿ßoò2bAGNbll?ïÙwOÓä?rÒLi>JÒ?K YÔ5R?JÅkY?oørEdP?qz×O ¥?ïWƒ¥ Ÿ?™÷ȝÓ?'ŽœØ–Ä"?ˆkYÞ«O?‡ŸDàL	?''Z0E2?î@³"A•÷?"¥¥nù'Ä?'+úLb?ƒÑ%\'ö?¢ñ0½ä±Ù?‹™­^Ê(?î*vJ"ý ?™ŽZÙçÓ¾?v%¡60g¡?x=¹<h?ª"ç3B‡?˜0_÷¿ó(?ïõh_Ÿ?RúÃw…êÝ?2ãSu,2?5­Å×ñß?Q[€ ý?P~ùDœ?ïÍEQ²"?yŽœûú½ñ?fÚk*ÏA0?hº²¶Þ:?kàBäÃÆä?q1™Ð0?ïSh³ÙÇî?xÛ!H*c?€º|$Ø_?mQº{ÐR?ŠkV֟‹*?p7y•J†?ïž>j&—ø?sÅïßYî?fÆ>Þ³?ZÙYÄÏ?'¾Õ廋P?pZÅ3~o5AGN3FGL J0836.3+2143@ih*Á	J,@@$ÓÀíÀ:K/ÉgeÀ;Ô¶JªH¿¥ŸtD¸{8@
†Ã(3P@†š@ˆ†L¿çZþÞdFH¿èð­&¿2¿çÙÔ5ˆ^¿Ó(^öQø¾AGNbcu?ïü«&´Ê¢?3xD5ÓÌÚ?&/Ɗ`€Š?%r9"AÐ?/Ò
ê¸È?+Í$‡~D8?ï®_ã%ºá?ˆË4V?qºÿEŸ	Y?i`…íu?wHÆ?|mÑpV³?ïOÀi‰}å?"ÝtD2zu?{ŸÇÏ@©@?jF$÷6$ü?Ž@¦1þ6?'ßäS<˜+?廬%š?}3ÏÝBѺ?Mû¡ùš?QÝ4üœ€L?"ÀΓ€¹?|8ó®Oj?ïý‡)Kö?`¾åÆ}YE?ff¾é"¸?AGR3-pÓ?(Z3©q_£?Xí	`&?ïâ³^;ʆ?d>¤sƒŽ?XÞ~] •?SMe¼Üå€?`Ýb`GK?]²Šw)?ï¬/#H?x
þS'˜?nÚÿ1CF?`Íþ‡Ñ6?zRþ©å~a?v_í$y?ïòBâ +?TÖâ=M?1­ÄËêh?)æ¨2 »ª?W5Og¦=P?S06³yPAGN3FGL J0836.5-2020@nsŸ‡ð$@([qàíìÀ9"ØC""À;¢Þ"umj?Ø[·Êßõ@ - ®@Û$¼"Û¿ècpÎQ宿鞡S!e*¿é ,W™;r¿ïýÁ\‰ÌPAGNfsrq?ï :?
~e?†'Øý`'-?zCÿ =?ziûCE5§?užà둭Ã?yߕj͋´?è™G#Áó?ļºrÆ$?ºnÁSÇÓ>?±ø/K#I?Àcƒ)"?À9Œ
1S¬?ìþ尕Öä?¢¾9JÊ5?©j×AkF?•—é@JóÄ?¦¦Í¸ôÂy?"‰<á$ /?ç5{ÛÔ¸»?°Œ¶ðu&%?ÄjÉÃ?©‹}]_ï?½€é ¦¥?¦tE¢e_?ïÙÝÖ×µ?qgïV‹>?i'zoi?hl½'E52?ZD,}SF?_,Kȋ`¥?íuãk—8?±¸{ñØc?¢FB â®Î?ž{{9mp?¦[†©öà§?¨ËK¹ÚW?î ¦Ø`B¥?Æ‰Y£?š»Ô-ÉyÍ?"ùø#ô™?'/PÇåÿ›?}ÜuPBÄ?í•çC#Hã?"ÛSÍY%?¦µáwúnŽ?Š=و»ß?Ÿ×T¤ÂΎ?X¾'_Y%AGN3FGL J0838.1-4615@p‹ƒÀ~à±À\ `ˆ+À8$›†ãàÀ9¼n9™~Â?öű:5¥@ï†<š?ÿϾúQ?c¿Ù:E E›¿ã3õƒ¥¿éµŒ©ÇG¿î¥x?V×þOTHERspp?ªRÑʁ|?«ÿnöâ†?Çyˆ#œß—?ÂBBÖÐlü?è|}9Å&C?ÄæïÝ6ì?Üzt\À—­?ÓkSëºx·?ÃQ-­jåZ?À.nKY'?ÙÜôËwè?Ð_‹¡<?Ì×áџM?±³¢Y±Ê?ÑM¤"?°~©7Ö¸?à#x¹‹b°?¶–-Xœ±ù?Á㝀¦P?»õ­+FÕ§?ºo¨"nP?±Z©ÙS?è9#Ž¿9Ö?ÂC»"sȂ?°¢èEü?±Ã\á'fw?Ç蚫ú?Å5ªÇ>my?èXàÒúJ?Ȗ ™¹¶+?äÒeÚò¡À?Ò²|ÔçÎ[?¾Ó¡Ó#þã?¾eæ=®"?ÍL—ª£y?ɵ7~`G?І³^??¯¸™ï<Õ?ÐnD{"`?¯Üç"%m?ßì&ž?´‹Èíçq
?Áè1º¾É?»j¦ðwÕW?Âð,¶ŸíN?©ù#Þìã?æÉèd`…Y?¾bÃÃñ1MIXED3FGL J0839.1-4739@pžæ?šIÃÀ#Á`]öÀ9¢t3®ƒÀ:ZQU]*?ñò÷c#f@âeæ9@®èŸf7B¿ÞŒ£çÑ5¿í°˜ƒïä)¿ìZ¾b¦¾?Ç¥}=OTHERspp?ÊðTí©L{?Ä¿CÚÙ®?ÁBϬêÈû?€zÙ?äó6ÙZú¢?ÍWa!\?镂ÿ2?Íó÷œaӍ?ì渚ü¨?¨4Æ=3¸?ÅìVúQ"?ʺÉÍz?ÓºtfËÅ?µ'?i2¯¼?̑+ÿë»®?±ÁŸÐ/üÊ?Ýüõâ£Vd?·§zÛLô#?åž"ë<z?Ȇaùš5K?Ž¯Æ±Éží?¥%ÀUy0?ÔE"½6?È]/8°SM?̃K:?ÊA<§6vp?¸ð3•k?¼'LdÌL8?åÛÛÕ9"?Σ¹Þ×?íØýUz¨?¿$»ÝL‡ÿ?ˆƒ7tò?¡ß#íi&??¬Oh¦ÿÛ?º>z'þª?àGÝcü\?¹
r[Ój•?ÄSX¨ÉÉs?¯w‡c³^?ÕHïÀAÏ?µ²öĺQ?êZ›…4»Q?ºÓ<±çF?"×ϱÄã¾?‹è'IèN?ÅHðì«~?ºÝµ× mMIXED3FGL J0839.5+0102@l!O?Ù3ã@8_L?s³VÀ9È[[piÀ;ďñz+??ò%ëú}·@<'è§HÚ@æ­àMˆ¿ºsçûž¾¿¿à‡Q¿ ¢ô¿äE|	w[¿ïÿ‹Z,$AGNfsrq?ïT£4;á?×¯ñùÑ?Ž±J8¯à?ªü§â°Ú?G"¤ŸÀÓ?BNþ>ö6?ï â?z¿?—böwôŒ?‹ ÅÊßh¯?†m[²Š)°?ŒYÁ¨±ƒ~?'toòú?çEì4@?²ÙèîÈHy?ÊÚFóY~v?°ÑܾŽD?°¿>E•?œÊu.Y?îœÇuC#?›¸¹'P?š ÞôvòÁ?"d<'"Ç?'F>öpæ?«š;ï´?ïº÷Ԟ?"BÎEşn?€¡6åÒÿ­?"NjŸÑÜ?;cj›¤?2æ^õ¼"T?ï"íÚ'm?…Ñ2™!¨?{ì†U	ß?yå"ÏÁ?yœŒ¡yœ?|WÂsRi!?éÎ<ZñŠ"?«÷7
??æD$§õ?¨vÀ¹V?¤ƒ)¿¼Ïò?•¤²J—2?ï–î| ë?xŒFMUï?ƒÑ\Z<?pŸÁŽ´²?iÌxx¤|?lä&Á×ÇAGN3FGL J0839.6+3538@gcôŸM¡@B>n¿Ñ;ÇÀ:w»"€^À;¾–ä•?ˁâmÈÛ@
íæšÔ,=?þÄl@šúÿÛijãà¿Ø)ÉMˆÁ¿Û§7á\•œ¿ã°UþdIAGNbll?ïèáï"îÎ?aB2åèu?G¨XH¹Ä)?D'n(2F?a3ú<¡bè?\6E°
!o?ï#¯‡[m?›0mÖÔ*?ŒÓXpÎW?'Kö´¸ë?Še:ÓvÆA?×Œ´Òܼ?ï3ôxì?‡Ñf€
Óù?‡QsØB`s?uïåžO5?"äîpzU?€ºìß>¤ã?í«Ô¬ë?—#/ûˆ[‹?–¶Èt:žé?‡«@:O)?©çPõzÌ?"åitåd†?ï÷µG^J?Haõ­ª·‹?1MûŒ"Š?.r±³à_?HƒæÎ$¹µ?CùE	ß¹?ïº	0€Pr?}²ŒÉg5?peây†¥ˆ?mM'ݝ?r•…%Táv?v^¸½¹C	?«h_?m£-y-f?w̐ç]ò?]Õç‹›_?€ë0©ÚÉ)?dÿhșËé?ïYߓ¬x?v煁|÷?ƒËN÷Ϥ×?f•Îk¯ç¿?…ïy¶ ?qPÄgEWýAGN3FGL J0839.6+1803@ióÿ`Ï‰@?ÁúàŽµÀ:g8Yã¡%À;Û²ìPö"¿ñ~n¸Œ@WÕé4-?þwæ Zé[?µ&Pƒ{H¿ß3pÍ?ð¿Ûÿ)w-ð¿±bÓkÄÁˆAGNbll?ïù'Öð£R?@×-åø_?0Íc›­IÛ?,K<̑SÝ?Aó`óÕa?9"êZÚ?ï±ðèàԗ?‰,´\÷#y?p y–Å?'ÍtTø=?vç|8Ó5¾?{…"…‰éb?ï)å®3ô=?…)0B@€ô?‡|x¹‰«?ypfŸ7"?Žlój/?{#V'É,?ïÈùçj»h?u0ßiZ(?Ï{Œ7
?#
z7Ôq?{#Î<ÁÝ?tåtû]æ†?ïü#ØTóÖ?2"îDÿú?"ôôXë¨?±Ôž\\Ü?5fÂXk?-wëù¯É?ïäLÓÒ£?e(Ú·j"³?W¼ø@³l[?S æ✿?_©aO0­Ý?^zûÎt£?ïêÔЦ?sÇùi¶?yôuB*Q¢?jÔM"Ï'?}– ï;¥?h6‹àÑð?ï÷쑟`i?HS¶ä|T>>ø;Ú)‰‹">ò¬#†°þã?O‹Ú5+®A?H)Õ°ŸS¶AGN3FGL J0840.8+1315@j›Ÿ˜·@>+?8$4À9¢Àøƒ3ýÀ;À
éh?ëz¿Ôäì@9Ua0r@¾Í­ð>¿â5JBï>¿èy$ÞÔÿⴛ<Ú«¿ïÿ¸ÕҍŠAGNssrq?ïøÁJ–.ß?M§%CqO?(ä­A½Y`?%«äÃÂùs?FÁª%Zϋ?KIÑðeƒ+?îú~øf?™
mæ99Å?»U¦Ü•p?‡ݼñþÚ?Ò"¦¯pŠ?".uU¹è;?î¡Q=²­?•fã$WA=?—}M9—ñç?‰å¹<?"X…ðu?‹×oÞ¢FÃ?îh@öa¾?*oDzf?˜E:Íc!?Žð›Nž I?š²§*Ór–?–'t³?ïû‰="l´?Tsµ‹êèÂ?%#9¼Ýý™?`KåîÉ?9$zxÒu,?T)'•?ïŠ"¡Ñ²¡?"ŒÜm?€[â
*§Ë?xuÜø'gM?z6ë@ûô?y"È-éÇ?ï/_M1Oó?"!Äñ˜%?Žx1šß?vú¹¬¢øu?…¯ûŒ$-?|R9Íl­?ï†gJ"*?{¡cùâÍ?"ÊÉâTd?p¨q9	P?s6ÓÆM2?r[R¬¸>ÒAGN3FGL J0841.3-3554@p
Ձ¥‡@
æ1ÀAyÀ8 TS>kvÀ:ðÓu]z/?òã(­"÷@tpȕ?ü:¿ë½Ô¿×¿¿¸èz¿Ö'´ƒ]v¿Ê`P¶6¿ÜòàèbªoAGNbcu?ïC½i‹?œ5e<š»?cO'Ù®t­?pû0ÿтÑ?•3#^x-?š!ûJ3­?çX&2La
?ÐèÎôL÷? 7{ª5í$?¢C»Æ´½?ΑˆJ‰2'?ÏËúÐýD?ë%ò4‡¾r?¯è|ALT?¡8Ú ç­?'#-ËÏ?¾4Nߌ?­NdºZR‰?ëu Žˆ÷é?¬ª¥îW/>?¨DN°ß?ŒÉ u	z$?ÀWÓA—5L?«¨E¼ŸC'?ïȺ1sY?Ó
9‰?P@Ã)¤?Yy3Ðk'¥?w'Â)МÝ?Œ	EwN-D?íŸd®D:[?¼C7*lBÒ?Œ7pyš?"·e=Ž¯D?®ûôCévÂ?·Ê;yEÅ?îVKP¶Pß?—ÈÐé¼ò?•P¢AÏQc?ŠhT5µ1?Ÿåó®Eʦ?'˜çÖkò?íñ/›à,?"¥Žf×ò½?"ê«ÂВ?R
2	ǽ?¦÷°·S¤ÿ?øÜ.ÆeJAGN3FGL J0841.4+7053@añ'à@A7E AYÀ8	³;+O9À;€æàtI~?ûÈ=ägF@i•šÜe@<ѯµÄ¿æ›BŒÓŸ¿ëŸÏW…g¿ëƏ¨Ì^à¿ëÆl:]@oAGNFSRQ?ïæÁ¬¡øÒ?g¾Z¹'F?d$<¼Éx?e'‰óDîå?DhYþGœã?H¾‡™Åç3?ï¹8biy
?€+ZÚh­?oÊ.WA]€?quùîL[?s~·¤r>Ð?v.¨ú«?ì¸4•;™'?¥-fª(éö?´´& ™6I?£'J,$õN?–(ÒÛO^œ?Žö…üÛ?ïñT–…=?k:Ÿé2ì¹?3›úG³`©?HÍDé²??XoÔ%ÀÀ?j5|6¥å?ïìë_×M|?`¥üTQ?_£ó›µÖü?^OKøêøˆ?:1Ó@®†?<Ó({Ÿ»?ï䤹)Ï?iÝ­üšHU?WÙg'<Ž?TêžxŠX?_óNî±î4?c7ÛU%V?ìÝaÌñW?¤s©ãß?³;ò='i?¢)Fëè€?—cýtm6Ð?'²ŠÄèÈ?ïý›ÐfÆo?F]JôÈý?$V–Ͻ?4V®¥~Ü?'°ÎðÂjé?CƒšRï	àAGN3FGL J0842.0-6055@qN9¿ß~€À&Ð[À6ãÀ9	füŽ[xÀ;z³Z4ÿ¼?ñ0èóžó¡@¾Ù>Js@ŸÑÀ§zƒ¿ã'»¢Fֿ嵊ÂÕìË¿àé4ü®^D¿í#ÞùÂqAGNbcu?ìkeÅ	g?¹Ob™ÌF?¯|Žþ?®÷	â,–?ª3' Š¡ö?©Ë«K´
­?åÍljŒ{?Ê%Ð…
Ž?¾Û'ªN4?¹}ùéAî?É\Ì&ù?Â×k%+ÍR?ëÇ¢#‰z›?¦h:ë¨?´ÛÁyùŠ? ˜ŠÏw?©Î['(à??—ďÖ;$]?ê({ º,?®o ¨¤Ëè?³ÝÄ©ãu?£ ëãâ?ºß e¿ç%?¦àF]N¾?îx֓ӏ'?«•¦Ã>QÌ?Ÿ¡y`3ß?¢!"2ÿ)?'ÑŒ-ÙÚ?šÂF|Š@ë?éýLAª¢ß?À–ñÒQ?´Ÿ©w3ó?®¬F¹[?»ùþHÅÁ–?´¹³­
Œ'?íãâT7S˜?™÷ý‰|\?¦N²Ë±Ô*?"s´ðœ'?–æOÚÒ¬²?‰z•Þ©7)?í¤IíèY?"î÷ŒA?¨|SÇ)),?‹jRù	æ?š…Ï5¨p‡?ŠÇÂ)ŽLAGN3FGL J0843.1-4546@pÏ`Z³«À{=ŸrÌ{À8¶Ôš÷g«À9ïg ù	l¿òŸXj¥:b@Í­ð>@D5¿æ+Å`qÚ¹¿é8"ѳ¼[¿ét5A*l»¿ÝrFnyZOTHERspp?Ã!/gC'"?¿œF‹ïPÊ?¹o-ž‡j?»2»éû†Ê?è	Îr5ÉÞ?ÆÖ{Èßh—?魂Š'òd?̖V¨5ò?˜5É´–)‹? uþ»°n?ÆC< oK½?Êoµ6'b?ÑÒ%:»×v?°jCœ‹19?Î<
—˜7š?´ü‡ôðF=?ßÓùx½?¸M\úuà)?âMŠ'É#~?Ëìô-u?BáÍ$Ú¤Ð?E4idg?Û[yóáäŒ?ËêF/dF§?¸@!œ÷‹×?µ©Ðà?Â	ôÀ±¶q?Åê*‰I?èu~œ4 é?ɦ¦+'á?íÌæ?ÀÐDGúã?…¤J¥O?'¬Ÿ‡y™?­éõƒx£?¼mÕ¤(?Ó~#û?±úâtÁØY?Íôӄ»«?²Ûf+æµB?݇Ïz¯§+?µ®;¿@>¬?åêÜ›Ýl?ÂþÓbƧL?88Ú£0¼?1bÈƘ:è?Ô$9•ÍÝ?ÂüƒåŽuàMIXED3FGL J0843.9+5311@d¢KZS3@CÒ_³Ä¾À:è>BZîÀ<‡ªƒÍ?¥sÀìa@UÍÕ
ˆð@ëõƒ¥¿æM¤_è•M¿ã‡:]N*¿Ú åÓ¾
¿ïÿ<!H"AGNbll?ï£YŽ'¨´?€§¬ÎróÌ?|²Ÿ¤Fƒ	?zÏ=­o`?q ™4'N"?ií«=ª¶E?è¾#m(³?Ƌ'ìڑå?ŀÔv¥?ÂÉ
âÿ`•?®xü;'?«ÜÆÕ±?먵¶…¸'?¨…—êNH?·Ê;ýûý?£É"TZùŠ?§; "eó?"¶X
ª"ñ?ì@Ì~ÑÊÁ?®•s
?²OóL,BB?ª%
ša.ˆ?§SQ|Bi?š6¨²?ïÜ0'?fÓ¸ky?f©ãóí¾ƒ?b¯µÈ(ï?ZŠÈåh?PÃ
4=0?흸	œ6?´pSC+ËK?ª£E|Ò\°?®îjÅPp?—sÒԆ|?šv¡–^?íÞþ꛿?˜>\¢'f¥?§'ü1?"7·µ
#Ê?–þŒâ
?ƒt助ÖÄ?ïð'ñ?‰"­I¼Æ÷?"ê2½&‹?"㻫Ü"?ï"ôS"x?v܋à·#AGN3FGL J0845.1-5458@qT@(äüÀéá€8ªÀ8µ|N/8À;G^X?éˆu¥@X8ü÷@[=ŸrÌ{¿ávý¨À[®¿å»ÒÿŒ¿á€o$Ç8¿éñd—ëTÞAGNbcu?æîǍ6¤?Áâká`¾Ã?Z‡Mõ?¸!‹ÜÓ¼;?Ä÷êZ¯×|?¹JBüüV?Å_`i2"É?ÂèšYnA?Ü\v* 1p?ÓÞTð®e?ØóÙ¡FŒ+?ÃÐc˜‰Vß?è=§t÷‡?°>¬;ì?½÷Ñ{eڃ?§/ªCô¶?À
yps'?£Æç'?Öÿ3§L_ª?µ¦óaނ²?ÓÄöþéCj?·ª;ݎ¬z?Õ;ÕZÝ=«?µ|FS",?íÏYD?­ÿ 5ne¨?¤t^ÿ=ê?ž¢beÜÅí?©Î¬mS7?£ûxB7æ?×swz¤¥«?Ê\uó]k|?ÖÁ6‹5?ÁÔÇ7a–?ÑËpNÐ%O?ÀЅÐMß?í"Eõœ? é}¥Á?¨z_Rß)?˜-?ê€ÛÀ?¥Ì_)®?'\À|/Ç?äPÂRumÀ?­ÙkY©åM?É0S*°"í?¦¶üoÁrÀ?Ō£‹yµ?¤®âز6MIXED3FGL J0846.7-0651@m,xßzN{@5Φ ™@À:©-‹S†À;Ãý…Ò<x¿‹GÿFô+@	 ¼c1@Ò[ßú¦û¿ävÿ¨r¿çêIf~u¿ç"Öì‹Y¿ïûõ-Wë¾AGNbll?ïàÌÿ«$?fÔ'7'¸?aIâ!GÎ?_G©B÷#ø?[gl?z?X¨ÏaŠp?í²"x¿ž*?­Ó~/Åe[?¦*}ónú?ÁJŠ(=?¥[íÝ*Í?¤æÚùŒþ"?íþ?S°‰Ô?–(UædÄ? ;FƒJt?ˆ¥—È–Ù·?ŸÁˆ…{þŸ?‹§,=ñ^D?êï;x7Zp?©Ë§L¤b9?´Nu'ü»?£=þ}ÉÚT?´7¯Þ¿? À?'™DW?ïðnx¿À†?U"î7eÒÚ?T9m¿à·?OŸÎÞj§?EÓBῶ®?@֝½ÈŽ?ï"ùà0W?™Ö•Üae?‹2Ê:rÙ?'h'|£ w?‹¤†=¹wo?"+&@ÓÒ?îåcåÌß?"0½"|ÉL?•\$<Lë?{ ppOþ+?‹î¾T³g?s‹ñfe^Ü?îȓI?Ü[?Œ,êÁ?Õø?"HÒiµIz?ƒc³ °Ñþ?'¤Äsv•?ƒVÎŹdAGN3FGL J0846.9-2336@nøeÿ£¹®@(i'¿°"˜À9	åQþÐUÀ;VZU¶ëº¿ä@$ýTBç@¯ôüåš@6ãtt¿â@")N>¿àö¸dq)õ¿ãÅ1˜±ð±¿·eÖÞôl¤AGNbll?ïã[ú6?i'÷;—M?FUŒ¢5·^?AF½$ _½?g¢'40?g(IJ»'?îùe›Æ?ª©]Íÿ?u#^ 'Ë?ƒ|Ø»¾íœ?›Štè©/
?©ÝÌ"ž_?îŽ	(ÙÏ%?˜'"".į?‰™áŸ	 ?}²üÌV˸? ¸õèøK?•q"–g?ﵸ^*Ù?PÍGÒïª?:ÀÅ9h²?@"øwí~X?›ÞEßÌó}?LAJmÏv?ï÷@‰•˜?Oj¯RMoN?4ìn…F3í?/U–7é?H‡¡vý²ä?JÀQöø†?ï¶,qo{Z?ˆµø ÂÖ?a²ƒØ?c!X¥À'?|]?yO:½?†
ß^'"?ï‰Ò1Âk?{ò<M,;?uы‰D¼?e.)M?'¢­ûä…?vûXquT?ïÐêÎÀlí?fì^Ó?¶?§×¨F˄?lr&¹Ë÷?wù$€}=?fÅÃC65œAGN3FGL J0847.1+1134@jî4 ½@>à•¿ðExÀ9¾Ñk—þÀ;x}›ö¿î|"eÞ^Î@oS"ºd?û؅_¥×ë?ïÍå=Sj¿Øg½¯ß']¿×ÑåÙkÊ1¿Ð'oO²ß€AGNbll?ïîG¸?:í?U¿×z‰‹À?Iڙ3q¥°?EoÛgá?VƒB¥Lb?MÏøž'$¬?ÑÔ?X#»B¢?räՊ'Û?'øF8ûŸu?|UãŽf©è?ƒæg‰26?îô1î9®ø?‰¼s¤—˜p?‹æ7êÃ|?{Ÿ3ÖT©?"õOÔ¿8?×hw˜?îÑmwôûŒ?'È­…7±?Iô~4*U?KPی‰þB?¢X~HÊ?'Ž"Ã}?ï÷Ùq\ö?GW>¯V
?6ð'ƒR H?;|¿VŠ*Ý?E!ñÁ6!±?=‹«ìø"?ï߅]fQ]?nº)ØÚ5?YˆÞo©µ?StÄîG	?c¶—lÖù?i´"'q?ïßfàè@?vN¦™Rá?~оÏT*À?pƒN†Ò=ä?€ŸÆ×Üʘ?h"]"ý|^?ï½T)¤X?pñ'7Ìû¿?*™'L:sÞ? pā¸"å?€@š "xŒ?pÜX|·cAGN3FGL J0849.1+6607@bY_í¦a@B8y@]¾!À9Ô"Nßa$À;ØgÕÒ/?ÄíSÜ\H@ä'áqI™@!ŸàZž¿Ú)ÙuÛ,¿á™ ù;Ò¿Ò"¦wgYo¿çáMž™AGNbll?ïû§pWÎ?:ùvÍfUt?02õcí?2º9^j?2ÅS¬†xƒ?,OwºT{?ïr°Ó‹ÇŽ?ˆß_·Ð°??÷
KP?uìhj¶ê?ƒXEîÏœ?"YÞ:v?rî×[?xªb,ہ?wê"dÂ?nçÔokcI?'­ïÉEi?pzý¶?ï4ÌÃgžJ?‹Z»fÉ?t
am{†?m~Äå$ð?"cÏQD<Ü?ˆ`C+ ?ïýAσ5?+ªÒØåN}?#oªˆª ? ­A҃ā?(sa8îR? ÿö›_?ïËü¢þGC?qÈ*¶ÂáE?g~«&=è'?[MÖÓ[?l"±å¼–?mažÞÃ?ïÀbþt\?n(ÔR†Û?lÁ(]Òþ?g¨p¢®ƒõ?qm왨&Š?`ƒ²Ë›~´?ïΝ!c|ý?i.}¤?c ãϧ?Pþ ô@ªý?mÁúñ)KÉ?dó½|AGN3FGL J0849.3+0458@kÏÿšÏú@<hÿƒ~À9Ùé¿KÛÀ;£Ö™Õ(¼¿Ì¬s"é@CŒxsÚ?ÿƒ3Ù'?ïÙ]KW
пãCUˆPN«¿ÚJ,Qº¿Ý]4wð–DAGNbll?ïÙcQÅ*Ó?kŠõ!ä±?Pdá­v?L}þ³h'ð?nšû¾Ü¯þ?fÀ£‡ýº~?ï`C%ˆiŠ?šF'C¼?'²âÑS?ŽNâ[íK#?…܃ºd^\?""áû^åÑ?î⍍`•?Œ£Tº^¹ˆ?ŠõOÞö¬*?{K´MH?–3¦bº;N?"_ž,š¢Œ?íP†@wŒ?¤'{&?}ÀãŠ~s£?xëÅZBŽÁ?³ŸÁdA{©?¤%Ab]Þ§?ïóW2–Ö?Rùbše"²?:W—¸ŸÔ?7Æ
*Ú?RËDg[)'?N'â<Àkm?ïÆ©Â(%…?|Áùy4?h	¨©Ht?m©Æ!‰Õé?p¦JæXé?{?åCtG?ï{åxE?w'n@º¯8?|_ae{Ôë?eì±})?'×	¥éÞ©?rìixÂD?ïf¼|jF?ƒ ãùÜÉÉ?c5¹xÊ?T]œ¹6E?Á¹H`–ï?'hAN&C)AGN3FGL J0849.5-2912@o"
ŸS @"vï`¥bÀ9†°>÷Œ"À;":]Éß³?ÙÉü	È£@-Æ	99²@ñ¿€3-¿âw"©Կ㆖O7JÅ¿Ö֙qM¬¿åÿ¥2AGNbcu?ïÌ»"3S?rà€L_§?Vª…Z3†w?Qu$¨T•'?s÷Í jÝ?pwSQ–_¥?ìßc`w?·h+$=nm?—y)M'k?–i"ý Ö?³)_ƒp?³ÍÉ 5y?îj›çti?"¶é =Ý?Ix©eé?|º™ÍPÀ4?¡TœÏÙòz?é!׳?ìc ‡ä)O?Ÿž<8d?•/bA‰O?ˆmëÄHi²?·œ/çx¹?œ7ÿy1+?ïó­Æėl?Pη²Û\?A†ª$¥6?:ìHøîg??OÂ:—'åÕ?Ip_	°8&?îúÛ&hÝ?£g.cþs?';So%"?"ÁašàÒ¤?—†ñvOgœ?¹1Ln¼£?ïrÃt+?xL{/?{·—#z0?hëH‰ä?…sm.-o7?q>]íà?îÕߘßèç?1øZ 0B?‹Éö°UZÁ?oÖ
,ü?—_GѾ?{PÈHœeAGN3FGL J0849.9-3540@pTÀ%@ùJŸ¶i3À8ýJh˜À;9©y
­Ù?äϳ?'@äSV>P@÷«ßla¨¿ã߃<yDZ¿áаd6`d¿èÌÕ÷vw3¿å%¡8/­~AGNbcu?ïåaH¼ª?a~ëòo²4?^cÆvÇ]?Z[ìÀ«'?Wz,¥P5:?Q›ˆf
2?í½ã'­'?µ'qõ‡?'®‡ꬩ?‰–™<°?¯v+Å"ê?³©NGªœ?î%bß—J?•¾á;i™"?–DÀå"C?…b 'BÅ4?¢‡qœý¸?²…±ì]?îÓ:»?"ÑÄLXoÄ?s8罿ï¿?qyÖ6T96? hr* V?"\߀¸à?ï÷ÝC×4?JþQ"?CÎw¦»zD?A¦'Œ¸/?@&@+¹?=‡0ä#ç?ïEØ[˜¤t?£ì·ù«þ?l'ErÊs?s2bÒTðv?"´«æÇI? øØuJÐv?ïM/8Ž?ƒ)ò°Ì½?'Ü=ԇd?uǍ7S†?‰Ý}èñÃ?{·b]êUB?ï³âô4"z?sF…4ü?a‹íL|a?Pœ­^>B?}HÆvµ?q¯'<¥ïAGN3FGL J0849.9+5108@dóM@$³>@C‹ßœ³*À8…JÿÓ?À;"2¨É¸E?ð;çҌªH@'øyxçÈ@Bsàwy‰¿áJÈ|ÊÅ¥¿ä"W¿â+}Aý®õ¿ìéº~wAGNNLSY1?ïÅÇây©²?'N‰†&g?{hË9ß~?'GI™ÖÄ?@…/"úë?7ó5AЅ?ï´þÿ|´?‡‹è?pbÇÀ´hº?ë`–Q?u-Ï[qe?x±ï;ð7?íq•A×L?¡ä«pô™K?­¾Ó¾B@M?že>\×ÓX?–bÖ+ê?‡"eK,zè?ïø#é¥[Ö?\BhBO)
?{ƈ>QØ?""(LRG?LÀá[ߒD?[âV.Zeb?ïâA­c>Ø?jáø•–íO?k2o@c?iXódý·Ò?56yô§S?3£#Güú?ïã‡TÙ»?hPrÓ;?YU=×v}ò?U¢À5íÔ?_œãÌõ?`o¤:?î¬M™n" ?"ÕLl"´?žß_H%bÚ?'•æ4;–»?‡-Û¤–a?yUq˜"ö?ïþʨÛ+	?/"®@ê×?ÃMöØ`?
Œ÷˜VXù?ÉFûóþ?,ù þ–ùAGN3FGL J0850.0+4855@eNù?ò^W@C£ïÿ×¼À8hìt2À;oÓ £äv?êxÛ¯iœ@Æûþ¿ö@vž_|s¿áœej¬¶¿âå0
ö¿åB™OœËR¿ã8íÉéåÚAGNbll@?ïü"S¤º?4	ljéìÌ?0X&ÂGN¯?-¸°9Æœ?&
¹ùÞ?!Z'Úv\?ïµµîÜ8?'ÂûÉT¿??o^±­^â×?qîÙ0Å/?uu¯ÕQGõ?yá•ÕÓP?ïHK‡¬ ÷?ˆï™kÖ¦?‡W®Ü"¢R?ƒ,'^Ø
?†•o*"¯ù?yMoݦq?ïØ£â•-q?wAç˒¥^?<7¼«ì?E(¸ï?qê'âóŽ-?vºU<ü—a?ïþ€Vã?&ñÿ¦|ðÓ?#}€ÈKY?!kíc%?UÂX³Æh?/¹³°Ã?ïä·þ<9?e"&<
¡?Wè'ðT©_?Tšæ—\?^§Û†ºøò?]ˆñMÜ?ï™ñ>= ?|½¶ÅQ•ã?{ŠµŒ¡ï?y€ª÷›E¬?wôRF¤¢2?gô[=/¹Á?ïù·µÆ1?Q
[ä©vª?%'Ä*òÁ?'†êÈ\}?Cú]ß?Pòm"RAGN3FGL J0850.2-1214@mÕ¥€Ãÿ@3‡aÿÏX˜À8#¢á@øÀ;'\Ôm*?öÄxWª‹Ú@C™DµÃ@R‹Ö7"§¿Þ+¹½âŠ_¿âÀûˆLV¿ä¹2X9Io¿èܟEðAGNfsrq?ïðû"'L&?UÂj:áÉM?U#aM½?R	ª×ç(Š?AÊïx•?CÓ¸äžw?ïµ;yäٚ?Ëeì™ø?ku¥ÔÔm×?l&V¯ýǶ?w§p)XGû?|+Ò´÷Ò¸?î‡ÕÓAí?™¶ºwñºS?™Ôcy_?'牍ïñ?•0â&ú`q?ŒÊœ þög?ïè=ƒª?p
ÃÓÐc?*‡ªp p?@$¦\@s?eÂiðª9´?o`–uÿ1ã?ï÷ƄÜ?GçR;(¿?I'šQñ0W?E†Œñãɋ?-QW)pv?&‰‡'6x?ïäÚ©É~?e-"gú…Û?V3}_˜?R¾P2ÞR?`Õ»þ²D?]½"Š; Ë?ï&ìg‰Û?Ž,vµÑÏ?Žn"ê)ÀH?" 6–¿õy?‡ÖgêŽ+?'C/A?ïû\µÖw?IWÄëâ{³?U¿
02?"Äðr86?=F
Qßú?Hd«"MAGN3FGL J0850.2+3500@g‹gk*@CBî¤ûÍÀ:—6JÿÀ;÷3I¨Q¿Ñ›>ÎË]@ÁläÚµ™?þ¼òÿçVf¿ë>rH"¿Å¯c)ü˜¿Ï",¹úì¿äÏ$;&OSAGNbll?ïöPæÕë?Lo[þoX?=/
àd»®?6;yi¢Ïÿ?Fó5µiÁ?Dµ}H¯c?ïdTc¬«?H>0‡õ<?'ƒˆèžÈÙ?…óð?"gp÷>Þ^?…+ìñD L?ïd[@ºÓ?†€ßvOU?†Ð´ ÌŒã?uýŸ".̖?"kL©É4?€I-·V?ï=Ù$m?ˆÆmÐ!œÜ?w¤²ýòÍP?rªµø¬Bù?'[®¿€?…¦s×*>?ïûO·ÖÏ
?54;õ¡Ù?*Y@S_è ?!X¢É?8U ©Y+?0XRBæä?ïΈ&ˆ2?q¯­hÁ¨?fÀ%Ø(`÷?_R
sR[b?j·³hr ?ltøÔ(gþ?ï~½j"-L?sfŒ!D?zó ôÄD?guÄäãæ?'×õªö?k\ïØ3G?ïя<§ì?e¹ëËú?ci0P'Š?Q÷,¹õÄ8?k¥°QX?`µhËO-AGN3FGL J0851.8+5531@d>—?·¥ô@Cx†¿¢AßÀ:2)ösDÀ<¢nTqq¿ý<ÒvYùq@ó!i1Fõ@½3@IFE¿ç«—SKà¿àædçn—¿ßI°¹¬ð ¿ìéìPS](AGNbll?ï͝e3¾ý?uõ†‡G¢K?v0ÓÚJ K?tãD'35?HËd‹{?IEØ̊ê?塚†0ÂQ?Jº	bì•?r6×j{$?pÑþ13g?y€åpÅ(€?ykʒ®˜'?î
¿Þ'?›‡Sô…	?¥æâª]ç?˜yi"p@?'Ú>Ò(À?",ZjqpU?ïÕðKúKØ?rJVCK?=l;8¬Hï?IÆ!ûÔí?s1LÄf
?q¬Òy¾–¬?ïÝQ8p£›?oÂ<.X%?ou$<pÙ½?nµ3?9Í'"Ø?6müªrä£?ïáw.¾7?hÛ[FQçâ?Yøí‡mu6?U%ø³•¤.?aŒZ nLÊ?bmÊìj?î½FTx'Y?""‰½Ã?òä¼í+ž?'^N¼?"È¡k‹n}?w¹ÍˆâÑÂ?ïú1®g ½?F÷¶ÿ×ñy?j|ò¸º?"‰Y5szÜ?EÇÀ¢œZ?FGƒàŽAGN3FGL J0852.6-5756@q5X ÕúÀ!ù€	$ÂÀ8иϿÆTÀ;Vóâ»K›?é¹òïÔ6@·÷¨˜@9ùŸ"®ž¿â3ªÏ¡éI¿æaBq>²¿äòŸ¿Îa¢¿æ*í;¾XAGNbcu?ïðH éÖ.?TÜÖÝ(Xô?AÍÝh¨"?<ƒ¢c2·?V‡ÏÿɄ²?PÕ;d9ÐX?흺¯­›ô?¶^ŠA:q'?ˆ¼{˜hf?ÆÖ¨=­R?¯õ6Tkë?´G€ƒY?îӃýq?‹¹àÆ?Œæ‰ZV?}ßŠ´åS?—;ÂEVÄ?'D2\è?îÅmÈII?–"7ÂÕv@?rÚäÅñ?jâ÷%üÂ?¡RÆéŒ_Å?–¢þ¿…‰?ïùL^h?@w¼m…ìð?4rt&\íO?/-1á¶0?@–K›Ýø?8dŸE}A?ï&d¿X2?¡'zn04P?td¸7P»?rßa¬Ç¹ˆ?–:§}å?Ÿ/F_Lü?ïŠ^.DÈ?rd-y§`(?y1—ŒÚ?hG,«¸?€ÜíWbÁ?ed²pÐٔ?ï¯þèÓ¾"?tÏ¢UÝ¥?dßtp?RHX[¦6è?}ÀÍá
?szR‹ÐôžAGN3FGL J0852.7-4631e@p§Ü_|gZ¿óº_y5À6£Æðù²À9Ú¯ÿ6¬d?߬÷šU×"@",dŒòl?ÿ6í棿ÝßtDJ‡¹¿äjñER¨¿â²à6áé¿Éx/fŸò#OTHERSNR?¸³ÿ×ì. ?·}–««ÿs?uuxÓR"Q?t˄fÄ<«?쾕DwÌ?¸'ìÃû&ƒ?Ø](hî›?Ó_õtã¾?¬‰.¯[À?¨i&«­›Ä?â,>Š²Ô‡?ÒÚI­H".?ɲžÓ],?²ŽÁÁ"Xæ?®1ŸŠ"?žÐ,Âo•~?窅au³-?³¨fýá6?Ùcù"G?Á#6}Œë?v†Æ/5°?|"wÄʯ?ã!lwU)±?Á.û¶DJ2?Ï²n'?Èý16·TÉ?'gÔ|¥â7?²«a`ν?线GíÄ-?ÉA˜%Ñî?áT=ï¦?ÔÊCAë7?«H÷̝?¤áÛâÂ?ÙôÜÁ£w?ÓJhOZíH?ÐDÏ.ô+®?²qî´òô%?µNÐ	
?¢2HL€ÿ?å3Õ.'†ø?´T6iÆ ?àx'xQº!?ÀÅP½ª?u'èùæLÜ?kÐ_Vç=G?Þ¸Ñl2œú?ÀÑLýùYbMIXED3FGL J0853.0-3654@p2*Ÿ{Zê@ÑÍÀ<ƅÀ9IÏQâJãÀ;C*3<m¿-|ð(@çúU:n@yÀšºV¿Þ[âòí¸¿Þ´<	œX¿ß…±.Ov¿âe `jAGNbcu?ᆵv¶ÑÊ?u>JªÔm–?f"šÝ79?`Xsìç?u^wºå¯H?q¢̳*?ëƒ`H±?DZMÏ?•½K^ÿèú?šV§gɤ
?¾x:#gc<?ÁK!Âٕ?íÂÛxGuœ?›ËÐX?˜AÑz"BX?†Ã­}÷ޑ?§±_»ªÐ?"f¾ïÍ)?ëy.¾jš?˜V¨]u´µ?‰cŒ»f}J?|Š`t"'o?À…9Y²?—Ôż"µ¬?ï餁ݘÖ?^=Ö¦"¢?NIͽjò2?F×ÕȽ8ä?]'üÑ¡B?Wåîü+?îÕÊm³
?©
"[Ž‡?{•ÝWT?"<¾
?žam Iý?¤ÜRç-¡#?ï14ý|†Ó?ƒœ…Ô56ò?…ŒCª*´ª?u[ô?Pü‰?Ž&|ö³–"?z(õ£¢àT?î‰zt‡³µ?~†?š€¼?ySÑŸd=?_|/‰"{?¤=ޑS ¥?|òSPÖM|AGN3FGL J0854.2+4408@fÀ‡D,@D	e4Ù&À:ô°ÿèÀ<Ü»W?ߚÖÌf0È@íÀÓg?ü󚜲ÿ¿ïþ˜˜s÷?ïí–@ž«§¿³'÷þm¿æô·µ8†"AGNbll?ïå6ò@µä?kDZõ²ZÄ?V
´BÅ%ÿ?YÂÍxx÷Š?_"gÅ?q{?c®fŠ©?é:»Öc5?É㧏{ˆ?ÄAƒÉßñ?Æ<2œpŸ¶?«N3xT.é?­OÙæ¡ñ?îšqý"Ø?"¡džx5?"RÚ~¢X–?‹0ÿqý­Ç?˜^åÈÚ'?‰œ5oDÿ?ìÓe,L´?´?¾[ðÁŸ?¶Œ"žÌ›?´R%4ï€?‹SԘ'?Œfœ$
Í?ïöl)/4‡?U°1ð?Ô?4µjVÛ̆?4"fòú[?Kô¦I:\Ç?S…´ÌK1?î0y1;®¤?±9ð'óŸ?¤L°Œ?«y0ZøÅ?'ÚÙ@RÊ`?'߆~Wök?ïP"ãö?"Õð菱?"×ñoάç?~Vpùâ	˜?‡ϙ1Ÿ?x\H¸ýùE?îôVD–n'?") 8Cc8?žt¢¡ý¦?"×?h¦›žKA?pDH_çZAGN3FGL J0854.8+2006@iÙÔ?u'@Aèä€G¸üÀ7'tvÊbÀ:ÕaèRdQ?óÙq±s*@ÜÉ܂wi@žåE¿|Ø¿Þ¤Sʋ·¿äL
2n¬¿â.V#Åyi¿å
•Þ½ÕAGNBLL?ïù1£ÕÌj??¥Xo¯¤s?+~dî™á ?+¡ƒ«¬#?DYÖ«‹î?8ðŠOMgá?ï‹ ‡Ÿq?}­iþ½?j—Ïe ?l˜+S—Œ?qnH7?\?t¨Të
Xo?ïTز?Šýj|à H?€^>ÐþfI?|iŽ_æÜÏ?ŠK5û'ó?"=»	É\÷?ïè.X?uö°'ÿé$?­ù0¦ÞÃ?-Lg"}ƒ?g0aÃ{¬ª?uá«ÛØYÑ?ïü9…mù¿?4yÀøLg?%'Ýé:í?#ßÚlË.O?3rdâÄs²?,­ûôS3º?ïåV"W¼?føHR^"‹?Vé·ÑT|G?S|w@o?^i!ÿ«A?a4€_ÀÀ´?ïÙ»ƒà[?}emçjx?xµ‡ØÇA÷?p'¸±XC`?€.Í.,ÊJ?vKAbo²?ïü"Aëª?BÞ~ù«•?	"J©{mÆ?€QTL¿?;ìf›~&'?BŽŸZmȧAGN3FGL J0855.2-0718@ma¿ "_ž@7SÎß̃ÒÀ:º$TÀ;ÅÔî~:?èäÄÛfÃ@ Ì@Šà@…#`,e¿áèyÛ°ŒÈ¿çq÷¦a {¿ë&þ¿ïñۙ2/lAGNbcu?ï<4F·''?—¨ÿÛEu%?ˆº
`G'?ŽØ	•Ïc?ˆ8á%§âæ?ˆÊÕ¹ ï%?â%d€8?Ç+_¹<æÕ?Õn—3M_?ăi8u3Ö?¹'áÔîE?·ÚÂì¥å?ìª,œ@=?ŸT‰ƒË?«wðKˆè½?"Ûé†}k?©åEíߑ×?'9'‰…ðÝ?Ø×<ïÁæ·?¶ÿM¶?w?àÊ*lKi?»…š¢ò́?¼lºí–	Ü?§ÿ¤ÎF˜—?ï¡®EÎw?£ekÄX?~l¥Š0¢?£Rnà¹?p¼7°pͪ?n%¼nXØ?ë()9Š:V?º1œo·ÈÚ?»8)7íé8?³ÓDgr'?§
ö¤¡/?¬r·ššýE?îSÕ#Ži?ŽÑ3è#4?ŸŒl©YQÁ?† QÏƯ?•øñóì¯?€n¡ã²õ?èI–¡í?¦e€Œ}2x?Ê"mfŒ'?¤ñ´C?G?¦>5̓âŽ?""OmøíMIXED3FGL J0856.5+2057@i¿¥_5½@B?l?Ä;.À9²E¯6¹ÐÀ;!¸·l¿ë;¯P @À7·Qex@|Ì¿`Ó¿çéO?Ù¿ãdÞKy¿âkt}UkA¿Ü-I~AGNbll?ïò‹a-Ӊ?R¾d0)‰(??b¢Ð&h?5ï±^¢;?S"·¯q¯?O붞-ߜ?ï°R
íL}?Œ†ëÔëM?p°œ¸BÐ?k|žTY!?w&^m"v÷?|
ÁtˆùÈ?ï%CÖïe~?†'1Á$?S?"´ˆy0ü?suý4U?'Q*âN5º?~ûGoô»?ï9ù>a˜?"åW?ÿ_Ì?HÜ{ôâZ?FSeDôQŒ?—ùëù>Ä?"‡ÍT;~?ïûãÚÊ*J?5ÍÜ8ë9?+¦¯ÀRÌ­?#¨I¬÷?3
Ó¸æ! ?/Îþ¡è­J?ïâW×
?f1'nßTË?Y§a@èÿ?RÖ5¢•hø?`ÔxbFW?`¡i"×T?礪FÀª?gkÞ¸Ä?rËÄ[œÛ?X#—stwé?yòEïƒÊ?\‡
ïê?ïÖÏ{d
¨?_Ê¡…À"?-¸HgW"? IڔE4`?sª€…Ê?^n"×"AGN3FGL J0856.7-1105@mÔ¾ Ìÿ"@5}c`!¨ÇÀ8Ku€µÀ;ºßd?ð5`ç÷J¥@Á©Æ˜@gUê¿Úfñ£N'¿àúÑ©Á*¿à>'D´Ý9¿äYìý¼%AGNbll?ïùh+?BQ'Óbo,?:ÑP'QDk?9ž:¨+?9íWsØ û?2Nv`ß?îL¼Î±?²åâ{€l?™ã+I_
?›ÄøSIQ?œœR]ONb?­Í4p­º?îõpå›OÒ?˜>LWKµ?ŒÑuk 'C?ƒ7î˔S?'é(˜½‹?ˆcÌzŽÞÍ?éß²Àå–{?­|¬ïyÚh?«ç¡r'¦?›zôJ¹8?Á‡LŸՑ?«(¹/Z?ïý;~uÄ?- u8{1î?()],à7Î?"aÜYµ˜M?$½>"Û?á7:¬óQ?ïK	p®?š§x>%
Ä?‡õzl·÷?ˆ®i;V8?…H>Ý	z?'Ê—Z¨º?ï"À²ÉQ©?}§t(¢?~èâ,/ˆÚ?vpã¦ÒÝ?~¶Ä‡äÒ[?póÞΝØ|?튈ü4ç?"ǀt¾ö?¡ø*¬M'³?ƒäŠ:֐?¥fìÄËà?bs×W6AGN3FGL J0858.1-1951@nÊ?þó†@0‹hß½jYÀ9N^¢LƂÀ;€ûŒ3€?æÙq/‡@Äf1¸3ä@³¢ ~e6¿å¼áÀ­bW¿ã8؊ßÜ8¿ê],¿.\<¿átùg=.'AGNbcu?ïü0J©$/?8¨Ku«µ?3™"ïñT?2ÐÏ
˨8?%È.žçŽ??)¾_kÅç`?ï'#ÌÁlÐ?WC"­@?pÉÖõ?mòß:uD?ƒp'Ú3mŽ?Œ°ìí4¾|?ï%`~½A·?ƒå'«_w†?†Þ
´@v?y2SÁ.i?ÉҎ±é?zš×ôð?ïY9DoE³?‰~&6ûˆ°?lùvžw?j[ÿ:ùGJ?'V¶»«vÃ?ˆK}"qÊ?ïþ$"ŸS?%rþ ö-?"î—rVða?fuL[R?žvL¾'?4^ÚVî?ïØV§?p¶÷¾áÿC?[O:üz?SyFsœüÆ?jBLgJµ?l¯€Œ?ï˜AóxÍ?rªZÐîž?xDÞ|…¶0?iIq^J6Ó?{šž"îog?fœLð%Cë?ïÜ"Ç?iQeºý<
?Uëpåeþ?I^•ßE=?hŠ´p'äÚ?eÝݛp:AGN3FGL J0858.1-3130@oô/ ê[S@"p@Õ³PÀ:Z­ã×À;Jaοõ5D°^,@â?j¤
¼?û³˜Þ³ª¿â8[¹íª›¿ãyù»Ã:'¿ÝÌ̀i?¤½Üfj:AGNbcu?ïi–؀N?"`i¥Ÿ²?;ô3Eô²Õ?9g7/§0ù?']n5¶ÇÝ?"5¨áé?î¢/Î,{è?®
{Âèo?v|ÏÑk?}€¼ÍTê?£
€ŽÕ_?¬L§Ì­Û?íÎUKi"u?›	–Z3¢ü?'ðÒ,át?¡ÛE'3€?ª"B2öŸ?–ô'ÕO*Ê?ïxŸ÷ís?‡w˨/j™?$ЙËÊä?fY¤
¦Z?ÜkwY?‡pèC¢vu?ïâÎâ"L´?l®V±éÐ?-'ÑJ(KÝ?&ª÷×U=ð?kWð©¹2ú?kd`ÖK?ï¨É£ëá?'g$ u
V?`¼PY²ïn?f¥Ú½©·?ž©ÿè`?5þÛÏ?ï:TšaÃ?'a©$ðÞ?€¶"˜†¡&?m
2ga0B?Z[lí|
?}6&ÃéB\?ïæ8¡º­ï?]ýL´ËŸ>ó‹+m&P>ñµÿç#dý?i H.÷Ë?]îŸÐ[ÄAGN3FGL J0859.1+6219@c%°_®¼A@C?'à°«À:RV	!òÀ<wJº8v¿íÒ=؆G@àc¶Þ£å@u‡_…K¯¿âÛ]ë‡fÖ¿ìąz¶?¿Æ>ôff3¿êÔeè´ÒAGNbll?ïó2Òu?f¿"ðق?H)#«÷Á?R@Xú³àü?Kz%à€?]]ºó<íV?ï}[tè+Å?Üáw;¼=?}esËtu,?ƒ†‹c
½N?öhÛÃV?…r?–"?íÊøüx'?ŸgqwhK¬?"lBsm
?'XìaYåŽ?©OÉ?›ôµNIòº?ïvhˆeÑ?†šÐúy›\?Uj¹-Dô?XÁþ)s'?Í®GY?…¾Å¾‰¿¼?ïðîß¾Žh?yÍöÄs1-?Lô=µ&ò?hó»™^¹[?OPCÌÞ|?l'ö¯>?ï×Uô-]?nÑe(×ò?bÍæ^Bÿ?[/WÝ£?eÜïËz Y?fæȍ¿¿?îÔª@¨32?"¼/â?‹&ˆ4T`ù?ŠSþGT¼?—×sÔ?D?Ø»jB‡?ïéîüá?_Ý÷CME?:¤m³R9æ?2e¤LÖE?c¨ƒë})0?]"Ø•ÏÖAGN3FGL J0902.4+2050@iÕ³ S\ž@Báj@ºˆÀ9Ñy÷ÜÀ;w˜³ÀŒM?ãjñÎÂxé@~<)Ñàˆ@Б_äA3¿Ô	V'
¿àDÚõ{äõ¿â
C	÷Æ¿áhCÄ×OAGNbll?ïý">tŸ?%Κ®ÂðÖ? 椰r¼?ÉDѨ?&×öúP"i?ç€üÍIí?ï‰oÓU8?Óúì¸u?z¿þ•ï+w?"¿½?€D?ï´üG?†8ìτ_?ïSä>aP?"~¸'….?'Õø	×?{>n—Ž°?ˆ0÷áÑÖG?z"äô?îìåÕ÷Ì?'fÒb‡
€?zäÕà¥Oc?rÌu)óÒt?›ªÂò³?'—"@–óø?ïþÇ9v)Ž?L6ƒ)Í?O¼Œ4$?(%Ôå?ÉÆ@%P?dú¶'?ïלläK?nŠpʁ
?bg³èÚ/p?\XÊGw!?eûàH›?h‰íà[à}?ï¡
©H°•?xãR¯¬(Þ?wÚ;ÜY?o4«Qh?xdÑ	Î-?qv6V•ñ>?ï¾#m(³?qAˆ©cém?f裪œ?R-ѝú.?uz=ñþl?oïÌLzAGN3FGL J0903.1+4649@e¢£¿ø¨ô@DÊ:?–îÄÀ:ªÐ"£À;þ>Ëí©¼ÀÈô>«·S@b{üû"@ꀿƒ
;¿å̪*éì ¿ê§B5sn&¿×ÏE%V¯B¿ïú´ù¾¿»AGNfsrq?ïÀZHÔbÌ?ƒ¢àstñ?W9{À"J?Yhà""?z|Ö.9=?¿y7±j™?ï‰8â¹aû?ëÑòe3?xy‹ëÞÆW?°Ö	'?u\À&?"‰bEäG?íQµ‹"ï?ŸQ^cÚè;?£‰
Ív‰?'}‹I‰[À?§[™~¢ºƒ?"ÎÇ	$¨?ﵖÉÊR¹?ˆ‰Rwç°7?.kQ`â½?IKÌ8Ä_?' Ÿi0ª÷?ˆ8ë.šo?ï和<Â\?fXÙÂnI?NOïpT•?J"ŠhÎì?bÙw¥ßë;?bQC˜Fåm?ïÙA™õ¬a?ŠÍv,‰È?`î[+a
?tnß߶¢×?eÐ
ÕS&–?ž™´J¸Ÿ?î‰ÚÊ;wû?ŽzYûE'?™ëø}
?"þÜ45÷?"ÙŸÅ·íˆ?€_xj…¾ö?ïô2Â[?fªÌâ'C+>ÖüZE)ÏP>ñ:YG{š?WªÏ‡ÌA~?f£X¸êsýAGN3FGL J0904.3+4240@fSÔà—"ì@Dña_–hÀ9øE~RÀ;åٚ:©I?و]·k;¸@j3óL"W@ο¿É?¿Ý2`Ov
¿ë¬Bn~¿áàʐÀW¿ãÖ–íAGNbcu?ïñ~µg«?Zfh[]p?@(n›W8?BŽx(I%v?Uæº
ß¡K?Uü(¶~Àô?ï"¼¸$«?œ[ÙBò…þ?Š«3ÎMPL?7æa£}?Œ¥ž2üÏ?"byxÊ?î©ËRÏ/Ô?Œ±…ø/L?‹úhçJ&•?xÌHXŒp«?œÉa7œ\>?†$äNJp?íÙ'd%¢?ŸO;Ói?–?µS‡²)?Œµ{9–«|?§M¯NQµ?š}5ð-Î:?ïüUBŸ?7k¥þÅ¯?"¾«ñ?!«­öD£í?6ö5×æ¿?3;QœªúÙ?ïÀ.e»h?|d~}1²?o­Ú»lç?pGŽ—W~þ?pL#À1²?r{–q-š?ï}w8	|?uèö#ˆ?wU3PøàŽ?_4s>®îî?"÷˜gd¿?r²†ž>íÅ?ïM§cî?}o_Ùa_0?€¦-¼Qۏ?h¼Q=Øþ1?~-}µ
)ú?u­d™àûÔAGN3FGL J0904.8-5734@qA¬à2ÛÀ! ßÞøHÀ8W,ˆõ¨À;.Ãø贊ÀBjØf@Tꙇ¸@›ÀSu¿æë!{r3œ¿â<>.äÄæ¿ãëË'(Ù¿ÞÿM»8êAGNbcu?ïòڃwKï?RãL&Zmñ?7iËôÖC?4ÆNœtF"?TfÞ·(b?PÚºq~?î'EtYf?«÷.lAJ?Œã³X.ƒ?ˆC½{s_?¢ú¡µuW?¨"6žâ(¶?îp%›VC?•ø¾-§Ìñ?ÄڎL?ùÏ7«Õì? ï"@m¸¨?'æD˔œ?ï"Å+­³?†
_¾ý7?Հ@¹&ÿ?O…b'!<?ŠïßÀR<¤?†Œ,¬Wù?ïúM¡…?>´w]²ø5?,¯5ÇpÌã?&kS'•?@UôËúg"?8æ܏q=Æ?ïxú€0´?™ÈQzâmu?iK'¼æéÄ?r'(†œm?‹¨¿(th?–ژ]ž?ïx`¹Ô!«?}¤Ë_½x?x÷]MW?jpü,æÜÑ?…l#`
¼?y!VSÇj?ï鐳®t?]³õ»[>ÙÜð|­^?i"aKö?fb^B£7+?]´$ùIX•AGN3FGL J0904.8-3516@p7߬£b@R ß´+À8¤ÌHBŽñÀ;NÞ̀Pó?çB4E,@Ž )֓@4TçÑá¿ä]ÅÀ¾÷w¿èQKòœÀ¿è	YQnÌU¿ëÉvBÉˈAGNbcu?ïïZùOõ?WÿêA¸î/?Pó96òZ?KØõu"vÁ?PVÔ¸ðåˆ?Læë´cš?í÷
Ãð}?±͜a'E?‡‡°«1†0?"GGyìI?ª­g¤ }›?®!	ûVx?îH…ÑvæÍ?•Oä=Ÿ*?šFKž?‹a‡2‡Ú?œ¨úÍ Ž)?‰|í·4&|?î]pãºF…?š¨xǵ·?‡ißwb?€9
¼Mó?¤A—Iê!?˜ÿ‹ÒdA?ïöÐf$³?J}¾a!	?H(X7Úâ?B¾ºçÚ
•?9U
º,ËL?9Ôü˜­¼?ïrh'8ø?Y¤Õð‰?p–´Â~è?j%˜6a?‹-Ë{z0?Œ¹é܂@o?ï/ö"ÖÈ4?†D
õ+Ó¨?Ž	PIê'?ÊBPS÷Æ?…ù
2;?r}9Z ?œÛ‡??zÌì?ùQ%?pé@ÂÞ!Œ?_)\ 5^?¡8r­ß†?xXÓk "AGN3FGL J0904.9+2739@hÎrà\̊@DE À:W%ô†O:À;å)äÕØ¿øĦf%Ï@
);}"@DßX¿¿èfŸ=ò2¿êqȜçVç¿à4>&}Ô¿æØÿsú3ôAGNfsrq?ïۗ[Yu›?s±~f*Œ?:¶¿ÿ+
?8AE\©[??pˆæjA
6?sóO?ïYØÿ¾š8?¯%౨{?ŠÐÒYk?š¶·þÐ?‰Ä¾¯iU?«Ã4fœ¿?í»p[²®>?™JïFÝ%?"#6>jÚ?€!קW"?ª·_$Ä(»?"Æ}.RC‡?ïLbFú˜ë?‰¬Ñ¬EóÉ?Q©QCÓ¸#?P¦ ù"Ÿ?•Y"±?ˆù"裝?ï÷~{ñ?Q>3:îª?%ôÒÓ¯À?%üö]Bw?LŠ`̊õ?O†fð,ˆ´?ïÔŚ‡ú?ˆúE? 
?bå8dY¡?pŠïqbNò?i €\Œ?-Œû-ŒÆ?ï0š>Û"?€CFhI8?€®_v¢'—?f°)Õó±M?'•ˆbƐ÷?|‡b]´»?ïâ²Ög¼c?^óyüD°p?&‡Cð;b?À½ë˜Ã?këPðWF[?^Œs)$¼AGN3FGL J0905.5+1358@jàÓ`Ð$p@AúQßƤ•À9öŸ..À;B̺XV¿Ç½úÏñ@"gtƒ_›?ýknî1÷?Á‹á.Gà¿Ü¼pá6Æ¿Ýĺ]€¿Ôš:YÔBôAGNbll?ïå‰HàæØ?a1i‡íš"?W2I[µQ?Ox+
?]»V"¡Œ&?X''ï–ÞL?ï~¤(úÜ;?"Ï øž?wÖ\it¥$?|%ÉP1ö?"kÇ}`Ê?Öm‡mb?îåAó6æ>?ÔÇm{S?8w"Ð?ƒÉ^Ç£O ?"»†'J?'â­*ŽR¢?í^šýÇÁu?œj­oz¼S?rz§íÈ?p_	G ×<?³ã}¿úX?œ+¹šª‹?ïöÈ:ä#ù?E‹Òqdo?BŒ¼ÍŒv'?9Éå¨?BRW¿Oñ?:»é`ºÅ?ïÓù;듌?ur¥iԀ†?buâGl×î?dC³Ú¼½?iá×þ[Ÿ?p¾GÚ"`~?ïlÏúv ?|ì•y(QÚ?ƒ̞Ԗñ?uš­—ïB?ß?i#?oX蔠?ïPZë€cŠ?}%{•o¹Ü?[ÖX9nŠô?H	‰øí›Å?"7=Ô$	?|¨{/'ñAGN3FGL J0906.3-0906@mËýàÖo
@8• ŽÀ9l'^;õzÀ;ƒ0"'¿ÀõTͯR@-Ñ4§@, šTU¿Öø±*"¿âû/–pšG¿ßi²·#¿ß:*šÐbAGNbll?ïíh`×?ZP9oŠ–å?Iåm\׊?D=
vTnP?X<‰fÒ7<?SÒ°¤­°?ï‡\ܦ§?'TGš‰?vEcm'í¥?sŠ»21?ƒXГc?Î­µuç:?ï.«l³e?‰¸ÿßu{??‡pI¹ébˆ?|$§÷w½ž?'b·,°?ƒ+¶P'N!?îžC0›7?'"]ªÙr?j'¡ÀhÀ%?c¾ð³·H?¤yRրn"?'H_ï#Æ?ïúþuÍs?;YÆ,|} ?4²³8f1u?(M/d;	?:­Y€ˆÞ	?4D¶°ùx?ïփW7õ:?sÁ4<AŸ?`Ò¸ï'D,?U·¥?_|j?h©ï̄ê?p""Ôº°¬?ï'i°·‡?xÆî?x«\áÁŸG?kpþå_«
?~Rîbhú?s—íÁ"?ï°x±	o?o
'å ?U¡ùÅja*?A^'f»1ý?-»©~³ù?n=%Ã:ª.AGN3FGL J0908.4-4916@pä˜à†8¿ñ(Hÿ"_{À8r.ÎI¤À:VZ°O¾"?ä³m»@ÚÍÉwê@"]60¿¿é'íø…Q¿ç׋—£J¿é÷a¿Þõ^®XÛPSRPSR?×1"mž¥?μùpì¶?©¾P?*×?¬ø¼ÐÖ?âã'9'Ø@?Єy)•-W?À–joàb¬?Å;@{y?¸Õ꟒ú?¹
ƒr®?è¿Â†³ôö?É/J"¦Q?҅šóz¥Q?µ ³LÊ\?ÃJü "?®Ã¹k°£?áõ Í®?ºmï¿',?Ô©øÃ0ýà?ÁG~óê·³?¡O%ØÜÄt?ž·0gØ«?ä–@çs9?Á·S±ál ?ä‰RQå¬?ϤHÁ‡@É?¡QÅjcé7?¤'ôš#à¸?ÔÃ"®DB?ϛIz¥ì?љ±Ùù¨o?Ðâ±Þè`Û?·K.
Ä?¯8îÅIF?äIÁQï`ö?ГñÁD®?àOÒºB?º/NpY?¼ÛşB6?¥ÀØ×)ï~?Øééj^ºî?·ñÂS
äÁ?ßãÁž£ø ?¾Å[?£0>Mú|?''Z–W""?ݶ=Øí[Q?½¿Åy¯¿MIXED3FGL J0909.0+2310@iŽŸ¾vÉ@Cö?µ!µÀ9š@€MÀ;`¹4i"¿ü
½áÍe@*ÏÝMy?û`àÀt¥¿å¥<Ê¿ä9÷;D"¿ª¹;9UÐÜ¿Ônô'¥AGNbll?ïüF÷O5?5Üwaì¿?ùëBaõe?®¹©à–Ü?9é
-Sm?4‰ÎèTŽ­?ï¯dÉ¥U?š>ЬGŸ?i·4¸+Ÿ?k…K`}ýˆ?{ré)à?™¾Y«½À?ïm
‡˜e<?}úKiė…?yߚÀBHM?pèù¤­²?‡Í²Ž^Ý?v˜(f,Ž?ïÖFÄƪ/?oVñ?$-‰>Ú´Ã|=>å˜u¢Õis?tÕðª}µ?oQO7?ïý}'¹?0ï Y¯`?åç\ø/ý?|×®aÊ?,5/è	‰p?,%QV]}?ïᔏă¨?|áäàä?Z[
SrC@?iòù'6Ø´?a=ë'À¶,?p ýZœ÷?ï¶ÉHo?r䚴Ͻ†?oSþP›­?lûÛA%'?tñxjÚEZ?gŠ©Jà¦?ï÷%E´À?BWÝò×Ã>Ì~(…'>Íj"oP]W?Q§5)}µâ?BPSdpœwAGN3FGL J0909.1+0121@lžj_"ÊÕ@>íÏ ¼£ŠÀ7Ø:ø‰À:Ì;ëh™?üj%
%É@uÔÔÙ
É@AÔÜ:Óæ¿ã'xµ•Åò¿æ–èžÜÆâ¿åFi÷óö¿î5 é¼iAGNfsrq?ïb~S±Ç¨?'wåk‰xÖ?2fÂrNÿ?ÈJ8L<?kîv7æ0?l"‹§Ré¬?ï†q¶aã?Š撘3î?|ª«ØÎ?zØÓÕ v¢?€QÎ,?'ìÆæ!">?뀯׍^è?©''á܎?¶Jh¢vz?¢Pÿu?«`1=ñše?È‹ÈÁ<…?îB†B­WD?¤góùõ??Ž3¿¸ Ê#?–¼;èµ÷Î?¤J«åj‹6?Ÿæ{/ÝN‹?ïh"‰-³?‹¯8éàÁ½?ES—é¡?‰I"ÜŒø?jÈ©ÕævÎ?jÊf$>1?ïÇZ\—Û~?uÔLc?k,ô'fú?c˜×¹êõ?mx¯\Û'?oIʸñ.É?ë£Íò^#C?¨¤µ•C`·?µhP±ªNÌ?¢Ù¡í18‹?ªòy\ã0?œÆ©áÕy?ïZˆžcq®?ˆÛó̺(?"`î™H?~Š
X¿ ÷?"üêY¢(?>#·GAGN3FGL J0909.6+0157@l_ 'á@?W°?ÎL)À8û̈Ú.µÀ:îÁðи?ÙÅc@0
¤@wœÄœR@T/ŸªÕ¬¿×ÀÁ`¤Ó¿è¡ ¹*zõ¿ãOÿô¹È0¿ïþÎSNusAGNbll?ïD4"l?—A¢±'7?vKnärY†?x{Gê'j?'éý¿pß4?"È+á÷§?î$¡7G¿Ý?§"
 yÎ÷?¡TeªA,?œle˜…ÿP?˜Ã
õû´? à.Ҝ?è'PZÁË?¯@8úÿW?µ¬^–ƒþ? ™¦Éq½K?ÃuiT"'S?«dîS?äÝKÛËÍ?²f¬¹JG?µùoeeï?¤€‡Q|ü(?ÐÇpž)?±v¡'?ïBœð?—¸£¡º?oE‰È#ng?yÊŒ]F±?"Þ´*[?'2‰Ô¥jP?ï"~€þ1?ž*Ucëª?\GçeÎh?•
F~4Py?†ÂPŠž÷?ƒ¸µ'd?ê¬6'h£?ª¬'H•ÜP?±€¾ñÕò?ž «–e??¹Yøñx?¥¦'ªýŠ©?êæQ a§î? >lìû1?§µ¹ÕŒ)"?'Zð4²™ƒ?¼òš.T@?œ6C%G!AGN3FGL J0909.8-0229@m9pޏ@=ìð{(À8Æ,p¡RËÀ;ƒ†.'ÊJ?øA¡^›@ŽßZn
 @"•úR¿ׯ"[ê¿å9Z£æa¿ãÏý‹RüI¿î'´m–—˜AGNfsrq?ï'bÒCjt?ŒûŠ¬?.V?†3'l"	?‹@ü¤Ÿ¿Ë?eЏÒSõû?bÊ D%[?ë~–Mß±×?¼"ZUƒb?¸7'X%¾¨?¸U«¨ƒÐ?§§vvè=?©'I͌6ñ?çó¥‹B™?±Û¹§¨'^?ÈJsšñ!Z?¯Þ'±¾ú?¯›Øäã8?žUeuNó?êS*ú!=?³³¹¬8̈?½"+V£ƒ[?¯ ÓºÝ?°D|ØÁî:?§e2‰ÀÂ?ï´{ä
Am?«|`´ë;?U-gÄðÂ?¥Ä¯Ÿyß=?Y³'ge¢A?‡yÑ
Ìd?ìÝðôÒØÞ?³`«øiU?±vӜaÚl?°Iþª)/?žf'í>B—?œ{y'~É)?éI‹º¼\›?¯ÅŠ'¨"O?Ħ"Â$°Â?«9RÓú?¨Í1G[ðR?™ž!‰T·n?헤]%?™‰7O6Cë?¯™
«=?–I$ÿAS?‹²Ï†Ìž?…´-`ä°êAGN3FGL J0910.5+3329@gã×@Än@E:íàBËWÀ9!þW‰TÀ;T4£u»n¿×,If»4@oÀ£ÉžD?ÿ¿/ •A?ßàÜn€fB¿åwuÂÏÈÖ¿Ý1i¿Øτ!¸6"AGNbll?ïø
ö~!?Tå9±KÄÔ?'Û¢èÞD?)°µÐzž—?IÝ><hÝ?RÕÈÇv ?ï¥y¹KÝñ?‡¾MW2?qË!4ƒÄ^?t†R—&?{x2›Æã?'å¦eïmî?ïëæÃmþ?þ"ŒJÇ?'YyÃI?z^n¬¥IÚ?"UƦ°?Š"u1²Ö?îº#Ž
ÖY?"`ø«\k?U;íLº9í?S°x·¼?£³ç³ÿ¤?"+Ö¾*W?ïý¬Y ìZ?:*½šC¸û?Ö=œŽ.u?îB$J¦?(OBùMµÒ?5ÕÖ,¡Í?ïỐÔ?kaõ	h?[
«ó?UqLhsà?`ñ?'$×?eºé‡?ïš×Ÿc³?|!Ú]¡Ã?v1'±sa?oÌÝA¥Ãõ?|b¸›ë?uF€}uïï?ï»DÌãõ?rªD¥Ç?:ƒŸ¨Ðy?/ì<ETï®?€Z¯ÉeÊï?qÖt•¸bAGN3FGL J0910.7+3858@fö@ÈG,@EÈ?ŸR@À:á6U&£À<]\Òhî?Á8Tú3@Vöï‹Ã?þè`§	Å¿àò
·'$?²'Ÿ¾2…¿áø@{+¿ÌhØÞ VDAGNbll?ïæ3|‡?eÿCÌqA?Z°S©Ò=?a*ÀRRù›?Xé†å4"1?T§:He%?ï~«ñØAl?'»(ÿ`om?€O¾'øª?‡ÊÂæ¬ãG?€ƒ½ZK?"1©àT2?î¬^¸û';?Ž¹°\ÌA?">^Û8½?‡äñ?—5Ê
|e?P¹Nh_?îÿο¹?"í(ä…
6?W´¬KvA?D<"¤?'qkåò±»?ˆiiGŽ¬M?ïø¹,@?GӞ™®¨)?3•l9Mp?4Xr€n?EúeÚéI6?BÍ$§r¢?ïؽK×?qÜ«1‡"?aoʹú?`'9ÇKTy?eÓù³Õðæ?j÷ûàoÆ©?ï_ʓ6©	?}bµícKy?ƒ¹,}'?xòÅn?"õ¡ÿ¯þ)?l…3°Wˆi?ïÉcEõ'¤?pÐ6<ë¬V?níû-ûÁM?câ	^àk?g®¾ßAK&?c©‡ ûêAGN3FGL J0910.9+2248@i¢Ÿ<pÊ@DƒڐÛÀ9'4èÀ;—;-C/?â=€á^K²@ŠT‰š"@É eϿ׋ͮt2¿ãtÂ6ñ®®¿çuᚌž¿ë_[XÑAGNfsrq?ï×CKŒÎä?q'jÃÓ?rÙ÷}ï?q6¡Ìã"?8M£¥müÃ?3³è°­ÁÝ?ï–èhgP?ÉÇòõ£?w#eæËÖ?ƒ ójÕæ?}Ó¦ÀԈ?‡Ð»?í­ð¹;'?Ÿ9·±?ªy£^X>Ê?š‡Õ¸3Á?•N¢[,O?‡ü[^4?ïb¢´AÝè?ŠÖPÎ…?v	¼[ñ?uU؝
3?ŒRt°ÅÉè?†®4OJ½?ïêv›½¶.?d%E'íºì?cäl^ŸÚ?c¸?2I?*O€o-qN?%1è…œŒ?ïÛ%›½X?r‰ÝÁÁÝ?`:&½Ã?[ԏ³—"­?dÂM3濙?kq|}׬²?î©¡©Tïé?•žc"
IÁ? [ÛN
(?":ý/Å>?"((fq;;?{#[È%d¾?ïßÊÇJ=!?caoш)?ZÉ4GH?I}ŽÛèÉ?c1Ô%>""?`ñ'cxIAGN3FGL J0911.8+3351@gÕ¦°)(@Ec—tüÀ:7‹dL°³À;™¤µVŽ'¿Ý/¬	Lž®@
bmÔï°ý@Ììš"ì¿î7á…ä¿«ÈMÙt¿à
_¿O®¿×ÏI_«cAGNbll?ïŒ?YÝ8'5ûi??Ó-ý–>?7y'-?ZÐ Œc
q?VùRãŽò'?¸Õ@†?ˆà.	šáØ?tÍ-‰<â"?uDìŽt$¨?}äuúô΂?ƒR:-M"?îâŠíýõ?‡:ä,Õö?ˆR¢)ÚÈ?ufð˜?—…l$¼.?½€Z¡m?ïphrÛ?‹ôófÒb‡?lùHû\C?f±Q
Î?šrÉÖ`9ö?‹"rµmú?ïúž?>cwˆÔU"?(ñx-Ž
|? âíIÔ?AoMeš€Î?:p"@Ùâ?ïÞk¢v?kù,Fšò?^—µ?Wyµ§Wúh?bæÔ$Ï×?eʙ·»´r?ïƒêt
Õ?p=dÀ;G?x*¿ÃNE?aæÚ\²Ô?'ð],Ï>‰?hKL¼"˜ð?ïÉaóºø9?e?àÆvíØ?R<…IZò?A2cõ'?v¿äÉN+G?cŽÞ¶¡j³AGN3FGL J0912.2+4126@fŠ¿ðEx@E«³ß•ý-À:_›q
.À;ÛßÞèX¿ÍÐU5¼@
:MXÎM@Ч ¿ê™'Îr‹°¿æ	7ÖÓXO¿èÕ5Ú"©?–sáÏwQAGNfsrq?ïþíE_§þ?'ânf?C«(´ç ?ã˜O$a?µyŒÎw@?Ÿ"êú?ïºl{1]?
ºü
TÄ?m«ržPã?no	Êòh¦?sô	H[Ú?uì‹4û*?ï[åù'?}¢‡ÙB›ð?€@(¸ï?rÁUÔ'Ÿ?‰A¿*¼?tœ:ßS$ÿ?ïäìÖØic?g±3JL'Ï? zC˜|'_?*¼§û,É?j…
;¦H?grFDæ™?ïÿhÁñ³?
•õÈ-t?Óþ³ÿA£>þÞ6`=S?ûx÷{(>ÿKôŽÆ,?ïæ>íjjò?es\Šñ¾O?WeŸÙ?Sž>l;ÛU?\"ÖvR?]\¾ück?ï¶\~Â9?cZ·Öû_Á?o‰ðê›bD?WÙñ¤½?uÈ8sÝ?Wø9cÙ+E?ïý{l¦?71Y'GÆE>ÿG=Á¿â)?´ªE_>m?5§±ŽÅ?6)ÃEáAGN3FGL J0912.2-6452@q£˜¿pÀ&~wÁ½oÀ:
ÑÒÆÀ;­QU])§?Ú±¿ë³@Óá:(@tߥíe¿ädùŸÕE¿êÐKÝN¿Ü|í¼[u¿êÏœ'r^OTHERglc?ïeƒ÷é'™?—'©"](ù?t…­ðé?{¨‰@ñåÉ?ŒP~4È»n?"Î	LMï?ì½ /Sm?·È>}i7Q?ŸœCì3²?›%èQJì?²¯s"Ý1?³w4ûñd?î¯\y}š?• ´èjè?¿fžØk?Šmý"nٖ?Ÿª­Ðù¦K?‰ûq°Óå?ì–(ý5††?¥L£†RK?˜zù°b?VB°=oÙ?µ/ùϱ¥÷?¡ˆy¾`b?ï¼»p•$¦?‰25^?e_­	™ùê?mAœmä}ü?vòqH0?"Ô =¾¸?î¨%‡'Ê·?¥¡(ÚïÄ+?‰nÃy‰PC?ˆŸ¿†9ÖÁ?žCíJÉ?¡>¶øcÏ>?ï5™úÈL?ƒ99ëß»«?ŒD}S*?r à ™?†~v¹«îí?q–Ãõ¼pæ?îíI-Š@¥?ƒoòÞÉ?`‰ª#¯§?t=¨óè?'¦•€…K"?{ü¤™ètúAGN3FGL J0912.4+2800@hÐ_ôö@DðãõhÍÀ:sḻôÚÀ;¥Á*[J?êpl÷м@¼™£Õˆ?ø¤¨¡s3?ïýð'
g¿å#º'ê»Ü¿ã!W:é?Übö¨œAGNbll?ïëBè¡®U?e‹«a›?M¥o ‹ ô?R Æ¸üUe?Z§w3ƒ\6?_ÅkÂ
?ï©ga°k?ŠŸªlà
?sv"'¬Á8?ƒ*´G9ŒS?wÕÊïŸW?~¨Wü"-?îQ½BÙç?™)¨‰»Cý?›ðRXªu'?'—½ØZx?™Ø
ۊ±ž?ŽQ;~R¸¬?îìF¥*òG? `úÌÒeš?mf™\.?'#N¢œþ?žÊX;EõY? ;K®ÊÆ?ïõªóDkü?UáC&­?Eâ¢_¦º?PE'÷ìÐs?Cr#]·®¦?CDïSž¸?ïá3·¤˜?md²º?XÀ(ÿœ–?V«å/qî?bl4L1¿?eúy§bT?îê÷þ:?•JàÑ8?
8ˆK?Š–
™d£?"6º_v?Ûºìə?ïÖâ[:Ÿt?tš.Z'‰?LàfxØ?^qÜλüþ?q
Ö5"Öù?r<Ö´ÿêAGN3FGL J0912.6-2757@oß<`Ÿ@+×n Ç‹DÀ9Ì(—ξÀ;—A<á?àÍåù;=@ƒhÄÍ$@"ö`o"¿êI:Û
$¿è–™*ø•í¿âV¬ƒ~¿Ýºfá¾ÿãAGNbcu?ïë£-'f²?fß®™¸z¿?NÔ©ïÇ?P" ÙBi?Y­;¨yi?doP÷êŠ?öÊ!L?¨÷¯ÖE?ˆ÷Õ¿>ä?×BÐÙO?ž²6´Í?¢ª"Ti§?îij†þÙ²?""{Œ8>'?Ž¤ðÊØ?zæ¡¿|?¡Ào]j?9©ÿIJ?íbYå›ó?¡GAó?nŒ
öå?ŒàÏZ"é?±K‡]™ó?… áRê?ïùª€Ç£?PŒ"i¥ðÉ?2ûZµ¹¿Q?:ˆÿŒá•??°Ÿˆæ\·?H1ÒQá­t?<ò>?‡]î'0Ä?mÍ#ýèþ?oolðÔI?JVÁ$ôf?'vº÷9"?ïqpÏ1<I?z&Rë+|ñ?{'‰Ãé?oÀ"$Ü?…â‡SƒÑ)?sì`%­á?ïP¾p,|¥?'ú*P¨
w?­óا8û?qÚöÒ?‹ùj	•`?|m-ÿ¼iAGN3FGL J0912.7+1556@j³|€"Þ@C)è°ºHÀ:dÛé*ÑÀ;><{±Q?ÛÐ?фË	@ïK"é!?õœkþÖµ.?䧸ò¿åÍY(¿ä¤ÖFE¶?æ«9åUAGNbll?ïç|¼Ž?fƒz¶Ž?>Mãó	£?C9);í|Õ?d¹µ¹ôÐ?eì#ÐLÝ¡?ï³!ï$KË?ˆ–« ×E_?pOâ°º?'º…#¢:ã?uß¹a&µÈ?yÿ«

û?î7Giöê?ž[ûnïÏ?¢«Â૲?˜êbswj?˜A'TW™e?ŒŒAѸm?ïYԄüÿp?™Uá¯-]?D¦ê1Ûóó?`/a¥ã1?" 8H°i?™=:I?ïîê¯òݔ?e37û?9\¢È¸Z@?8
%ȇ«?[Ówšðù~?dÙûaõ8]?ïæ";è‹?daš—ðž?V·¢Ke?TB:Ïy%?\"m Àn?[‰"š{ï?î+'ËKð?¡ß\ΪM?£AÚË%?·Uz&?"…"ëÇ¡°?%"z{?ïëË©ûÖ?mtøˑb
?$1íÄ	%Á?;€ßçéÉ?c±¤ë{ö?lïO±!*AGN3FGL J0912.9-2104@o3b¯È°@2zeÀN9IÀ9.66òÀ;Uv<?A¿×Í.E|z¿@«%󄜇?ÿä~ð ¿ã°ïÄsŒë¿àõíSļø¿Øõ@gô¿à¨&¿AGNbll?ïñ»·³5?Q+ýq<?D"'ÏGM?:Š°Ïhu?RxÕ£è×_?K!b‹;±J?ïlWpn÷?™°Š»ŸË?weüät?tfŠ˔?‰`pæĆ?–‹¶¬úÊa?ïxÿ½‡W?‰3½ílò ?‡»\±pƒ?xg1z?"31ÿ®*Þ?'–5K½I?íåQtÅW?"?cRC–?gJÑ
¼ê¡?`Ë
?°.ìzݯ?"É'ð~»n?ïúK³\¹>?9€,ƒ<E6?3RäÕê!?(ŸÍä^5?:O~½øMA?2¦Ö…"DÜ?ïтۀÞ|?x›fãÓC?aMø%'C?Wv]Zö/?m/,`Ù¦#?t¦†î*ì?DEev?rã_´'.Ë?yÒ$óÒç˜?f~Í07ç?á8ú¨iI?hd*š?ïlã§Éw?tµz"e¶?Vœ¾Îò•Ù?Câ"•^Ãi?'·¢7/¿?ta=Q®AGN3FGL J0915.0+5844@cŸVŸI@D¬à f§ÕÀ:®…à19À<%çbzH›¿íªf@%ßã@ÄÊ7J3@ڝ`˜¿ä%Š9eŽ¿Þ$Žq¿­L¿ë†k‰2e¥¿á錐òAGNbcu?í…}¶lÂ?ÆÁEîTd?¶RÓç'.?ƺ•rm…¿?rx÷~ˆ8?€`ãéŽ?ïgVÑH?…{Âv»%ä?tµp±¹6?rd9¬DO9?|–ãò±J?yVJ4c?팚
`_?§/'DÈ´?¯ÎÍcQ‡?¥ŒÐ"5¬?Ÿ']'\í?ŠÔÇkY­U?ï¡õ`Ï_?€\±¦¿"?e€l³ÜM?eý›þw
?'"Gþ¹/?}v•'¯Ü?ëµîÞ^^t?Óêk§ô·?ÀÍ«"®?ÓÏ$¹PvÄ?f¦YÜpO?'2e¡Ó!?ïۍO3ní?nûú°âj×?`'LÖ?æ?]BEÆBúè?dTyB¿?f4jq1&?î—Ñ«-ë¡?—Ýî[ˆ~ú? 4žU0­?–E5ΟÞù?‰šÂ´Q,?x/Ò]1íº?ïóKSíñ?Wü§&?1º¹¿?%ù²#ë­?U%oºÃ,?V ß{'¢AGN3FGL J0915.8+2933@h"žà*w£@Ewa_–hÀ8yœÇ]!À;ãÙq÷¿ÕF¾1­«@!B"ãÒ?þFA,ðú¿ÜÙ{ÞêþÞ¿Ûçª\-2¿Þ{å†#'y¿×+jš8âAGNbll?ïæÀýo&?aGÂ0ñu]?U_bEÚQ³?P"8t¿Ö?]¤:áR?V¿©÷~\í?ӄˆ!?'E
3%@?x㙀ŽÂ?ƒ@Iýh5Ê?Çü§/­5?‹CÚᒠ?îoó5ŸÓ?"<9=Ϟ'?ŽíLç<Ï9?Go'z
?œÛ[*Õ?ŽÙÓXr«ñ?ìÅ$C΃S?£W›'àE?v©†yøÎ?rݟü‰ÑÄ?¸lEøÛ?£+ü%]2?ïõ8˜;ºZ?l5Íø‰ÿŸ?A@ËA]~?6µs뙝?IÜÓs@"~?k÷"/sæÐ?ïÖû(C¯Ç?tî8ÉÊ`?bswÛ~¢e?aê–çÅ?f'`M6u?nd3yˆ»Ô?ïNƒ»áÂþ?"
@ð2?'Ö—·Ï¦?xRë O¨Î?‰ˆyÜpöç?|¶ñóêŸN?ï=»P4?ƒ‡d
ˆ?\ïÒÂLn­?L.2²/PV?›ÉQ#Pj?ƒ¨ÏÛAGN3FGL J0916.3+3857@fø{€©Þ‹@FÁ?À:qGZ1¤¾À;ð¨á59ž?ádû3ßÍÓ@ZáZxq@Ùhy?í[éTlê¿ã¾grJ~¿êÃa›³¿â~¨ÜŽAGNfsrq?ïãuîïŒ?kQ1®øHJ?i-Ðü:_?j<ʶõ'?>
Æá³èó?8Tj«¨ ?îÿ2UÕ@?ªvxÐW?‡ŸvFf?Ÿ¶ Ä8?UåŸ2‰
?¡…œß
?î@דȀ?—¤Ìôv? ÄédÄ6?"Z݀«	y?—µƒÒTm?"¥",Oòº?ë4§‡Ìp9?´âŒj(?µØ²a8?'?¯žÞÿ‰ n?°'b£?¬ª*ãè?ï÷í"z ?R¸3û3U?L—Å\¶?Qeß?܈?-ÂÐØöªÚ?&˜V~¥Z…?ï¸2‹î`E?‡ž"õA•?qé#î½O'?~ã®`/%—?qý–Ó}È?|mUZ²Î~?ï#
»½'`?ˆ‰ÚǧÃ?Ê¼7tŽ?ƒ¦ýM?‡r"Ù&³"?z‰ûa‹d?ïiKYUî?¶Z.D—ý?'êÖ/hå?ƒÐ<‹K?…»N¼?…ƺ›<BAGN3FGL J0917.3-0344@mfˆ_Js@=äÀ_×,À:d7EçjÞÀ;²ȼœÔ¿ïµbXBiå@mó‹R"?ü7ë¿+N¿é8}RÈO¿×9[B"Dã¿ã–>¢@öÚ?¶ºÚM
AGNbcu?ïõâ8€
c?L~}_º?0okçˆã?(çr'À½?P´¨ÅP	?IÿP…±1?︑†G#Í?TN.Þ¡?nNðvÊ?oE«öàfô?tw•~PÉ?vYN'ÀÓ?ï0–+·$*?'|^Ö?†ãÊÖ¸?uëŽ"NÖ?Ö'þŒæÂ?u²Tö,d³?ï¸iÆm7;?z|~酎L?§Çõ¡Xè?'…¥‰*U-?°>ÙP"?zu¿0jH¤?ïü[ÁOs¹?5{ïoýÿv?~Tè?U5h
?5'v•^–?2ò²ñà6V?ïä+>®LÀ?dç"ïÓÇo?WR0µ8¶G?SߊŸ=a?`+©3U?]Üþ;6dO?Eéæ…?r~U['I??xVXa½?lõµl'‰?}OÊêõW?c¼À&TŠ<?ïóôAc€6?N»`Øñã>úÒÀó‡~¥>øH'㲑?W¬1´F…Ù?NN…¼WAGN3FGL J0920.9+4442@eö*?K@Fg€iFëÀ7ƒLŒ ŒÓÀ;6K\äÈ?üÏ͍'ùg@â$Læc@ž–Íar6¿àÎ"Ž[‰$¿å0ðÎ3Õ¿æôc6'§¿êUYyK£öAGNfsrq?ïÖ֓•?q²ÉÊzÚ?pÖüɐ<"?q8½Æ¨{?MíÌé) ?Hé‡ÎÚì?ïÁ¢ÏDá?}1mùì4X?m‡â4XC?n[Ïß{Ñ?pjÉ}#b?t4»4¨5	?í*þA©B?¥TNàވ©?°ÀT…/­¬?¢Ù2–A?—žåÏKXù?'"Š%/?ïô¿ÎÃ†?h¥G{ØQ/?)|¦v`é?FšÜŽ{Æ}?SPßU5r›?gŒX3äÜ(?ïȝß_²©?«êg9?i{ÈA²…Ù?e(ãnï›?mæXK]û?«Îô¼¢U?ïè2'ç·?cÕEjŽn?V`ßY
'µ?T‰…Ï10ó?Y;¼×5?X¦Ç¶'»Ñ?î<£Ým ?ž(ö^å•P?¤Ÿtšž¶Á?™No‡sèŠ?ŽY6B«M?ŠÝ1×Ã?ïþ?b¸Ô???z°éRÚl?
°¸}gð?$í$­?%]£à©Z*?>"8ï6AGN3FGL J0921.0-2258@oŒ¨€QÉ÷@2¥`À:Í~	ZõÀ;ÐNË?.?ðVGšs^G@Òܚu6¹?øÙì€nF¿îØ]Ø´s¿ïÿY<ÛÞ?ïÿd3Rµ&?‹VD"ÍéAGNbcu?ïÄ÷"á¬X?"9ƒ:ÑÈ?ISSƒ]üÿ?RÉMý<ï?zZ;§?ƒ'pÊ%O0?y¶>/?«x¶-Ш?pkú>:ôV?pâ,
Ü­Ý?‡ är£!?«Kü™ùMÐ?ì⢊a â?¢0íåt"#?¡©é",?'Âe ÞJb?°#¸–ßÖ?œÕa*n;è?ïEnQÊ×?ªŽ[Ú¾ŸZ?XkÑz}"ì?2"ƒ[ß?šð•Äé?ªaƒùU^/?ïÖ"ƒ¯w?}Ì- ¼¼s?MQ¦…B?Q"t1¦N\?qD¾ÖÖð?{ŒZ[ê?ïØà²:'æ?"íý#Vœ?Z/–?wÝ?S—AŸb~v?j6&X]}?ƒÚPÀ 9Ü?í´Ý¡u? bõH»†?•B³•–o?Š1É´f?ªÌ¿+Ì?žTçÑá?ïÝ:†5?yé@'»·Ð?WcсTÓ?l"—†së?g4܋õ¬Á?pš‰¤F*cAGN3FGL J0921.8+6215@cúâ~@D'¿ó vÀ8݂ßBñÀ;ÏùrGE9?çþRåÄÚ)@ñÚbâx[@–sßË­¿âxõ7'«Ê¿æÀ¯e2ߦ¿å4eè'%1¿ê
,ZÉGAGNfsrq?ïø9˜Z²Ý?Lò̓ä?Ei=±Þ?Eå‰ÓêJÊ?4iv'G?7Ï»mJÙ?)Òä?'$pP4?|D
¦Œ??…n+ÒwÎÇ?€»ð-:zï?"œ¢¶ÄdÙ?ï.ºŽ9qÄ?†§Áþ­¿?‡ýÒ¥À±?¤ŠÊÜû?ŒS‰¾%Q?|&áÁªÛ?ïqã"õÍ?Œž€œÖ?xDf]>`ï?r²b'd`?‡dëžz5?‰($8"ï?ïú¾2]ÓÎ?a‹N.4'o??÷tÈ$?Y÷YՔµš?$-óJ¤øZ?Bªƒ²'?ïÑï›{=…?q­S¬m»S?e"Ìe~Ëì?[™ðá¼äq?h{˜>à?lPD(ÌÆ?ï|ä'îlÁ?'"ˆ
9
¬?ƒI£»p(é?€™ðªRr?zú¤ W©­?l»lŽYÛ¥?ïãGÇî?m¡­ì
Jt?[Á¶'NÈ?R¶}4ˆ?]°;ú[–?i|õ8™¬AGN3FGL J0922.4-0529@m¶<ßï¿@@=èKŸ:ÃJÀ9°)3ÕðbÀ;±m'ª'?¸djÛ£@£ûùá@Y ÿ~û´¿ä&B×7¿×§¨%"¤¿ãÃÍZøZ¿âÏ1,·‡ÛAGNfsrq?ïùoðî?AÊ^²>"-?2qo˜ ¦2?,֌٭×?BeBE1G?;ØÏ2Yy?ïs3‰Db?"–
in?{NC~µµ«?së!é`3£?…"Q[<f¹?'clf#®-?ïOãg)?‰HҍÉ/H?€ßÂìÐ؈?vöRür?‹Z6¦[ÿ?"<›5«Ö"?îëO¡J_l?ŽhÅ×´3-?àyä²Æ‹?qÑø½	ðù?šíUUæ?‹Ô«»í?泥öíô?·T°f§¹I?nÀØÃ!?£Ÿ}6ÌÍ?|͘ìvér?±r~u!?ïтÿyGj?tÅ…?c_–†íÑ?ZÿñhÀºA?kjB—ÀÙ?qg€ð
ð?ﬥ^و?|ªì)ÛÀ?qxü¼ŽÇ?m3Ò£"à?x4v
e?x;Cfž?ï¿|8¤{?o'á".w?d"1OÇ?KØ°º¿âö?uÿÊù''œ?m?NƒøpàAGN3FGL J0922.8-3959@p•É 'RT@ѿÀ9ŽaêÖ£À;n©›o\¯¿ð`ëeU@8¶*@žlŸ~"¿ë@†NÒ寿ãÃ¥×?—p¿ëõØùù"8¿]Í­"Å–ÅAGNbcu?ïËæüV…Ñ?t¬²ìy?l¶Ÿëî}-?m&9«ù?gbcäQZ?cû‰&órs?îAhPVZ?µ‹°È–N?y•,£}BS?¾O·m"?¨¶Ùóá?Ÿ?´+VG™Îq?í¡BÇi¥O?šg^?ÆZ?›‹ŽTq:c?ˆ''h‰2?¨&^Q&á?"9U±ïC?ïfû'þÞ©?‰ñîÑKºþ?4W¸_¤™?DÉYÈÌ?'Ï3ez[¥?‰¾G܊{?ïì ÝZ¹Š?bªX¶&üo?T»äÍ털?[û´…'¦?R`!é·Ò?PŽOˆ±Ct?ïÍÍA«‹?•x5aYãÖ?b¥OyŸ²?fq5"Á¥7?‡ã8ޓª´?"|'©Ž¤á?ïvÍÍäá?…ê±Õž¯7?ˆ†Ãƒ@õe?y‹%¥y´?íč9ï"?ßhiK¢.?ïæ1ÿ§?^çܯÛ/Õ?pÏ:Cæ@?Ë£üò6©?i®
¸íQ:?^Éc…é=AGN3FGL J0923.1+3853@füÜ@W@F´ a3÷À9Ï¥ôïpÀ;Ðbƒ'Öß?×â
ˆçg$@:–n*@,À'wé¿ê¦×>ã!¿æ±ÁäÄíP'•
¶	¿ïþiWVAGNbcu?ïðc&3?fȆõݧ7?R†ºúQg?^à¹?Jd–ˆ«˜¸?T'$Ñ|O(?îSÖ²1sž?¦	âçGJ¸?Ìv ÿ»?–qkF,ܘ?—¸³Ÿ±	? Èf›÷_ ?îú­_
Š?ŠÄ£Í9Â?'ë
_r?'F:UøQ?Ò+jîµ?ãÓ§B×?ê²5WƒR8?°æÂÒòš?¿p"¶ð[?°Nçþ-LQ?¥ü›_Ê?œ£¸}uÒ?ïíür+ì?sî¦Ð/¡?Xö'0€8½?lQ…R=¦0?IÖêî/?Z'"4z©?$5êH?…6!v³•¸?€Î#gwÙ7?~GîËñ?zž&÷.­å?{Œ«€<†?ïVX9@z?€Su¢¶O:?‰:ÕÝÐQÓ?v¢†~'Ñ?/(G)Õ?uÚb"_6?ïŗ=7³?ˆhwªa?•maüK?€•¯"ƕ?'7¿rÓ?}¯ÛpAGN3FGL J0923.3+4127@f‡Ù!…Æ@F·>À//˜À9cöHòÀ;ȉ¬¼Œ?ßϙ'2@äNô"Í@	3€
&u¿Ü'èJñY¹¿ä–'˜ôX,¿äèZÄFÁ¿ä¬£b¬XÊAGNfsrq?ïúkÇVô·?Cþm0GK?4¦ðRÿî?3Ê8~€5Î?8Ÿ+ܜì?@"E¨à?ï•GW'rá?‰ŠS?=
Å?xávÜç?we·<ó»?}[r¥p?ƒb£*í_"?ïO²ÅR??#ù.?'÷í[¾dÑ?vۇœZW?‰'8Äp?tQÁ<m"?ï4sóþÑ?Ç•¨i?|í—hTÍ?pMq­OÛ?'6¥4óÌ?‹$«oª¾Í?ïý }Ÿ¤1?-/)bÀ?#mÁû"]?"}ˆ¾Ž"{?"g¹ýÂÀ˜? '¡/kÇ×?ïØoVÏð?q»úõ°—÷?aœ>È9U'?Z9ìI7¬?fEQøTá?l™Òi»Ð¼?ï°Q,©'q?nè:U×?r¾3™?ðœ?hF¯Ñ¼8<?u62ó•?^e•ejXˆ?ïØ5;©¬ë?i™ ö¹;?aUÖî.1o?IcÒðn?ftíi"»Ø?f¾iUÛ´AGN3FGL J0924.0+2816@hÛZÀ?ö@F7¿Ý/ñÀ9Æúû´@åÀ;àÂ=&Ò¿êƒ
^Ü7@LÒõÛ¹Ð@^`§"¿å³|ZÍ	¿èÁ­cÈHÑ¿äV&²h¿Ô¿ä™°…™\ˆAGNfsrq?ïþã"õ?/Û·;5<?÷K(Pæ‰?	f¹žiâ?*#ñø'Ü?.4SzÙ?ï¾ÌÒè+?Q¬™žEª?jb›èÀ©—?lÇ1¬œ<ù?shH'<")?vaFMð?ïhs£Þ
‰?wÀ€ú"v?vúâ`'#õ?bRä\Ãä?Še¥ä:-¢?sO\GHOå?ïï>=l5ø?_¶@¥-?
`¨þ(e?
SDŸüo?`L@
Ï:?_"qiR?ïÿ	{"õ?!IQd³aœ?:úc{¿I?'™Þm‰?>®¦Ð"ô?ià‡tõ?ïè7'´a?e>̺}?UœRÖñyº?S2?Þ^dû?Yô§æÈ#U?]½øá´?︾?ҙ?fJ†ìé?j±ënÔA1?]
cÕbS¤?vGꢐ+8?_¿ù‹¹àv?ïýÛM6®?4KÍ9K¡Ç>íR×
U˜Î>ê؇"ôø?0;~•Šv?3û·Ö^>AGN3FGL J0924.2+0534@l\
á'6@B'"à4êÀ9ߔãQsÀ;¼Tdc¿¶¸¤®c@,ÁL#å@q·€	z¨¿âwˆ¦Ç¿í3m³À>ý¿½Ç¡Р¿Ø~.ð"ŽSAGNbll?ïóác²¬æ?[Å5únã¼?.¸" `!?1«Í¤D?Tf5µ_Åþ?Y\§JŠ§?שּׁßz,?'Ì ¢ˆf?q%}&¯?lÔY˜?x"(†pð?|ݔåbW?î³£-lâ?¶³¤ÀeÍ?ƒ£Ö'_ù?r®àÆ.n?Ÿ¹¯O«·?Ø²!kY?ïb%›èJÏ?ŽFø7Ö?J>óPRt­?WîЍë¾?'éTæãٗ?Ž+‹=O?ïûköô·?>
OT¹r›? Þ8zɝ?"ßñÀO_!?<1G²Þo{?9.Ϊe?ïß<ó?A"?hՂUh½Þ?\jïäF?V"ïrÑõ?b"¿žr¾?bi«B¶?ïv±¨?~#ï=Â?r·M*"°?YӒ‰'?‰­áÀ­?|Ü/P…•Š?ïã¥Àï@?cÛà¸}d¤?B÷[5ÖA?8M
uB?gÕï†LK?b›
"5¯>AGN3FGL J0925.6+5959@cZV`^åi@Eu@ýAÀ:¢,nóÓ¢À;öÓ)ÞÛ?¾']Ç»"@PûSóÈ?úq™ O–@¿ïÿ½Îc?ïù\•W?­¿Ô¯$Æ3¿ÉÝTâãîAGNbll?ïû˜qrÖY?8´ˆ'T¿?!wätZ`ú?¡'7ÙÒ?:€"	Àê?4<"ü5â?ï†VÔ?›o÷²õ"f?y,X©´vÄ?~qA6Ý0û?è'Iôã¾?—–œE›?ïS±ôÀlþ?|{hƅèd?€ýþE²;"?lתe⏄?Š""Ñm@?sÅV‹4Î?ר¦…?'¤téáÛ}?wvʺwB?uû2Ñ­?{EÉkvú?zk®õ*tØ?ïýÅ?*òŽ¿½Ø•?ƒN•U¶?/z*i3?0êokªWÏ?%Z‡<n?ïØ8
Á`?Xu-×?`çâ	oth?f'¨Ás¶?fàÿåCŠ?u¿¾Z?ï¡U®ªš?j0¡ÉlÊ?tÏt$¡Å?bž‹‰Ÿ?z¤a{m?_Í°	Ž\?ïéÉV6‡?["!ó"Äc?Xޞ%ƒhô?N.ÖÙîz?S+¡'gí?Qv/e€áAGN3FGL J0925.7+3129@hO8`™Ë@F«×à&EåÀ:å? §?uÀ<"6;%oü¿ÄXI÷RÕ@9.oÜ?ÿõ÷áMR¿ßù¥»ïb'¿ç>¥Ã¯¨á¿ºø
é˜é¿æÍXðýAGNbll?ïÝî_ï~Ó?†é³žŽ²?Q%U™­?tèۘŽùû?iI´Q_}?{2bKéŽ?ïšô°k˜*?…ܐs±ü³?véBw<ƒ.?t'w0?»:?{œeGø¨ ?€öÚȧ
÷?1+q?"iý/ý.û?'Þ66å;?ˆ¨ä{šI%?›P#¢Õ)(?r3k÷§?ï{‡çý?ƒü×+ lÇ?_Ð3Vh\?c2>'§m?ˆ§3þ7½?ÓN^™P¼?ïõƒ×æ[?qÒ?n²?=BYÆsj?q8üÕ	þx?M@ÄýÙ?NÐü;A~?ïÛg4A¦?n›±‡±¦?a§þ&"Š?\7BZÃ?bñ¶îîz'?fŽ2öàç?ïS}úµ?†év}C?'Ü	x"ó?»£†aÁW?ˆ_rÄR0Î?€œáM6I?ïé¾jœ?\뛨À8¢?PÑJx²¸á?FgøŘÛ?[²œžÖu:?Wh	fI¢ÄAGN3FGL J0926.3+5409@dM…@FA-@F	Øà†8À:°ÄŸá§À<'ªoª²Ç¿Ü¿¡26«Z@À§8¾o@£¿bV¿Ö[A?÷x¿åuœ#âˆK¿ß2̜ț¿ä÷)攅DAGNbll?ïö|bôca?M»)[߄†?A	œÓ*m3?C¶¢øí®ñ?EØ ·??U¬Œÿ³?ÊlÓÆ?…"/Ô/?s	j-	"O?sØژa"?{2°³éàZ?'õUê(?öVo?`ÁÁõÊ?'ՁMï¤?»gå?ˆ4e΄ì?rn3õd?ï§kÚ¢+?}‰i£m:?W˜icàëä?R¤‡g¸?ƒ1ü1(hí?{b|îxN?ïýY†rå?3¿y3ØA? ð#uØà@?%¹ÞH'¬è?)wtyVl?%Ñî7
m?ïá'§†8¶?jA"{Þ¯?[¸ëd0?Vð_È^ê?`ûã*ÿ'~?cõý±:Üà?ïƒl.4"?ƒÌO:Ü
?ƒ}ŠÃ0¢z?ƒÈ<Œ#Ã?wNçÖÕň?_3\ïî³?ïñ§*Yxu?TglT§!?<}xÙ­>‹?*y³•,CH?U'M"¹?Rµ\,΂–AGN3FGL J0927.9-2037@ovýç!@5kjК¸À9 ~¶¿DNÀ;»Ý:ZM?ݗ¿.©‹ª@çk›¦ÿ@ìßfØQ¿Ý@º–z'¿çVá®ä¸¿æþš­ÉZ¿æ¿þ½à ¿AGNfsrq?ïü7ᘶÆ?2‹¢ µº?.~9ÐeÐH?)áĶ9?.®?eyž?%_õËTë?ïŸZ)ÛàU?Œ°˜èƒ?tj'öp?'J¶Á¢i"?|@€á*i˜?ƒ±DU''?ï?vÍ^9"?ݘŸ81ý?ƒz4·µ>?rŠÔà7§Ó?Œ¨áž)?u!jl+'?ï Gœø?ƒHËËc°?Y¥1ÁXÑY?S &Kþ5?"ÄWùµ9è?'ÇÅˬ‰\?ïþWµYÏ»?!s‡Å‡bM?ÿC7Ï	?H!»5QL?
üš½?="Y«?ïܙY¾ôX?oH²(z«?\íPrUªN?U©éÆLn?dïþ€úž?i1×è©L?ï©^YÛ5?mˆˆy‡'?s~[,î?cÄ¿_kh`?x:vG&Ԅ?cåÈTí?ïî`êÀA"?]D¸7ß«?Ddj#û
‹?3‡ÎZá`ú?Yõ03š?Zõmv™CAGN3FGL J0928.5+4048@f¤4?¢­?@G5Ôÿ¡5oÀ:¦xmÏç4À;ø˜‡Jâ|¿¬»t3Ž<@
y$nŸDÿ?ýz¹>ÐuN?æèæ˜ðI¿Ìú\ßÌPH¿á+9/²±T¿ÄÔ+j*ÚäAGNbll?ï誀ia?c	Wf%?F†æK'߃?DWß=|]*?a³ÆÔT?^¢ôLõ§d?ï¯Wpv¬ý?'*mG"T?qÎüÒvùg?sr jÃí$?v…JÙuXC?z>
ëDÃê?îÌçyÌIÅ?ŽüB)qó ?Ž‡%82?€gšÌ}$L?—_Í-
sM?†ŒSu£?ïC驧XÊ?'aió'w?qKÝf¤?rHX}Rbº?"/Ӊ'Ò?®¶
"e?ï¾Ëõ·Q»?´ü0"uÝ
?-e*Å*‹?'zJ1ô5?®ÛÏæÞú?´ýY~î¿Þ?ïâ#ïjÔ?f»)…	<³?["×%*XÜ?UQpYˆM?`Rpºyh?`cøѤ)@?ïo³õŒ?y"éͦHú?~Ê Ôt¬'?m†'çB?"­²_¡Þ?s؜;šíÐ?ïâZO½O?e…ŠÌ×É?P`Oµw‰?Dܕöü¶??e¢Kw€GÂ?b¿ÒØt/AGN3FGL J0928.7+7300@akO¿ÆT
@Bwa_–hÀ:z²YƒÿÔÀ<
Մ+sK?ä\PZáM@
¨œÕä"ª@T¼ù›¿îeó%•Õ"¿ÚR#îò''¿ã'Å&W$¿éOÆD{
AGNbcu?ï¶5#Mb	?…:¤‡,†P?~ž §FT?"`5d°Â¢?YM5u-?W£¢'¬·y?ìëKŽ&|t?´²ž˜}?®NÿǔâL?®´¥ ¤Tý?¢üGYròm?¦E×ãqÎ?íl.>#H§?Jí"¡´?£1בÂx?"a¨¾/
$?¦(êGñ?"ë+OE?êNh	Ñî?²è#Y¨;>?Áµ´>ä†?°Î¦/*ð,?¤B®ãC5ÿ?šïû¸äÐ?ïäô£ß?vßÓéba?e+9²…Ñ?tÜÅòtÈp?K
õì<â&?Qßbeúª†?ï=é1˜?''Sª%?ŒN^·åAà?ˆŠ ©£ë?"l&ðîK?…uhєv‰?îúœà¼?ž¹yv?¾š>Œ?‡G5L&Å?Û"[‰`?}þ¨mñî?î>ý#à8?–~$Ø?§õŎpïÍ?'²¸8;ê?€¡*y| ì?|]ýîw&[AGN3FGL J0928.9-3530@ppŸS @&xwàâ-‡À9Yp×ÙpIÀ;ˆÛýÂ8?¬í9ŒÙ@
Ööz°@>5_³Cå¿ê)ýêÑðx¿æB]ÌJ,/¿àF–½Š¿éÎÁb‹eAGNbcu?íO9âàñƒ?²OÕÁ˜/D?Ÿ"?º•2?Uš?«BAöë3?­r">ˆH[?è€B>°ü?ȹTàW@?¶ój/¨`?³ÈpsÒ×ö?…B{
ôa?ÂÅø?êýè£"Ê?¨Î^>}?¬¬9g&k)?—<§'
×q?¹ºž6ŒY?£XêÌù?芞¨Õª?±	ÛÇ4´?³6;âØrŠ?¢eð¼ï?Ä<ϔ'iÑ?­vu&m‰
?ïJ^)¶?¡l#¼3'?4Rbcz‹?€™'Úÿ­,?ŒDÖŠ…Ü?žû¦Ñ{ãD?íkkÇ,™?¸>Ó-ò©?¡ãÆgu3?¯§"$"°?§f/Å £<?¬E–~…aÁ?î]>šœ3?"5>ÞߊD?—­EøüŽX?ˆ)á›~Å?œªæ¾¨E?‡N ï%+?í®Sق#?•D	ãÇÂ?œÈPíg?"s˜d£‹:?¦¶šdÓeÙ?´ý¨AGN3FGL J0929.4+5013@dõߨq¤@F¹!¬ˆŠÀ9.$I‹dMÀ;7p¯•"?¿káÝL™-@ñxŠ|E@Pàc, ¿ãI&¢ßœ¿ä㹺e/ô¿ãþ 2K<û¿Í½dqfAGNbll?ïüÏ¢¦CÝ?)Az;"ºA?µŒ¨?Œùk¨?á?5¬I}' Ô?(@8`Š›?ï´jݾ?'%ápÖy?nÒ¬$«™î?n&ÝÙGV?va¨
;,?}Vð›–Æl?ï'ÿséè?yP'uY?u»{	ýn?ddϑ8ÿ%?"bee‹{C?t­Ë¡é?ä|Z³?ƒL"$t?P±%b—Ë?S¿¬¿?Š;¢'
´>?'ýÿȖ=	?ïþaü®ø?"(«§÷?韮«ò?¼Ócª?!åÙ´[ŠO?å«úØÊk?ïâ÷3Ü.?kf'¶–9?XßRàön?U	Þ+Ge?`™"¦ø¸?eÀU!b?ïÀ3؅ÎÈ?c1­PË?jbîL"g9?R6ÞZá'?r´œ¤ìw?\EÏI?ïëÏ¢GƜ?_²$ýPÓK?7&0D`÷Ø?09'ú+s?aK—{ÜÃ.?^o±*ê@NAGN3FGL J0930.0+4951@e§€w‰¤@FÐ<aNÏÀ:h÷´×ãÀ; õ§·iŽ?çê¾±kž@ðÜ¡›?÷&€®ç	¿ÔâªÂêSy?ï…Þ7¿å²6ĕÏ=?Ý\–æ®A¿AGNbll?ïi¬óØC<?™Ÿî>ÙÑå?bh©Übº?dº‰rìÆç?}LE£¯9?™kß.ö£æ?ï/+DZ?"]\!uö?tL¶Ix#
?ƒðÐa}°œ?}³ô‰H?ˆ6dRƒé?í' ÉÏ~?ž^=Æ`?¤ð‡³`?—+?hžñ?¡ýlR¾²»?'³¾ïûŒ?î"3›Z[c?®Îs x›?˜þùC¸?­h|ÈÖݘ?"š"Qœxô?—©ãž'ú?ï´"5×IË?¨= qåv?P¿r(þ?WžŸL?€ß"7ò/"?•®Ìˆc¤?ïâº/û?k'%úS?YñçG§%u?Ué+VÍJ?`ñRDpÊO?f&ë²Ü,Ü?î5Ì-s3\?Ÿq†]°<ý?¡[0î®u©?˜—hp¬»?–o?5?h# †,[?ïÈàL94?xû«7ËÑ)?j¦pYfÉ?qX µÒ"H?lyCL€Ã&?oêjL'AGN3FGL J0930.2+8612@_'‡aˆ±@=ƒ¬ßÇ{TÀ8õ̏+\À;¥÷´#ì?äCÄeþ•$@,1â%O@xF€B²¿ÙúA©\t¿âœ‹ó1e¿å"Lu¿á\b'áÚAGNbll?ïû-³˜?;[Ñbþ'S?0\"†-ÿ?*ZÏK5qÿ?6ÂÁj#â?4†0€?ïaî üÇ3?—÷î
J‹Þ?€˜4Xÿ†?ô[d?†ìCk¬ÏÁ?"¶ór'Â?ï6lÆ|э?†Ükwގ	?†º€ÌÇà?~lAøÂüÄ?‹ªNS½DÙ?|n¸À‰q%?î{³6›?±÷?ŒœoEWÚ?ƒÖøGÃnÅ?¡°­ñæ?›kM½oÌ?ïý¡®‡*?)¦ÝÚã?#eëèˆ×=?åreñ?"4™´ÏZ?4—·"?ïÅ¿4çEý?|}á5œ:z?iÖ¿Œð2?giÀµÕ ï?p5ùǵ>?vA£ÖJÛ?ï¤×¦M9Í?qŽÈ!BÎ?vp2èiœ5?jc÷E!?f?w#ùêE;?c.$•ˆ€?ï±	2XÃ?w¹^ñ&G?qvt…sÖì?]nÚÇÂçé?ví¾_¦?sØâ"m?AGN3FGL J0930.9-1904@o^à?pX@6÷Û ¥&–À:‡âÀT†À;ȋfÐïq?ñuõjzÈ@
>ä'åp2?ý—sŸ4
N?ï‡HvÞ¦?ïj#hÿŒ¬¿ÙÞÏuÀîÀ¿é"KaiýPSRPSR?îãóL"V‰?¡KŒ¹ïø?'ÊÑâC²?•s3±Z?¶ÅhCO$?"ÃiûH?Óòi$Âé/?ÐÙÈØ:X?â@6çÑ=¨?Ñms"-ô§?¾4¤2µðù?¿øÏÛ±'f?ê2Ñ­‹ô?²"xÔ·?¸Â½ÿOb?¨ýœ«ûNž?µ¦´—ô>[?¦H?í}]?Ô/)a*ðÍ?Åt¯ÎÓüÜ?äÖHÀ§ê.?ÆYBsds?¡"(ì)Öµ?£R5\ý2Ð?ï6 'A?¤ZÔp†Û?Š/W>Qà£?–À®¯¡?ˆ(£V>¢"?ŸdN=š¬?ß s*͑¡?Ñ%þHè®?ÛÁˆå±?Ð;ÞËÛhÏ?´x¼»¦˜?±aC5
®?í=êv"h'?¢â~{"d?©K-‰KØ?›–BÈ$?¢Ö+tE?"ǝ*K?æhC$0Ñ?»³6	ªD?Ҍx:ñò?»oÔèéÓ?"ks偮Ô?‡sՈàMIXED3FGL J0934.1+3933@fÝ]¿Î·‰@GÅ)ßÍZ'À:&æQÙ¨À;õ¯}0­G?ê·ûקFU@Žµ‹è@8RÝk¿Ý¥ø³ÁŸ-¿á¢¹䏿ãhśwŒ¡¿ìÿÊKÏGAGNbll?éF9¥	±§?Ä#9'¥Ñ?ÉæÒ¿L}ÿ?Ãøú2
¿!?€j̓HG?xØr|8$?çõ=¦²:?¬èÝ4à?Çú±GÇP?¾·j(×~p?°aÄ´ú?®AÃ0tb?茽–à
?²‰8ÐxuT?Æ¥Ô™¶?°©½ ?¬ Bh_"?•(£.» Ê?æ`'<:?³T˜1ZX?Љ"1Ççú?±ŽøPR5©?«påKlç"? ƒ."q'?ë7<V6\L?½úPWu ­?ÁãÓ!ƒ;?½¹lâp<?ƒó¸iSƒÈ?ƒ]çܦÿ?íiþJëƒ?¦1éz5-è?­¢½¿õ–?£Qb$5µ?—z»&
i?"ôø9§?ì&'ƒzÉJ?¤ˆ~(Ï×ï?·+…ìùÏ?¡&6võú?ž—åºYƒ?ˆbü~µ"?ìOÁcŠ‹?õàá9'ß?ºô£;À?˜|'¾–ñ?‹—Ž0î?…ÚÏÉö;ƒAGN3FGL J0939.2-1732@oe'@š$@9v·¿õMõÀ9Ÿlr"À;§þ#†íÅ?ëÉï"Å@ß@V‡7Â9 @(Nß·
C¿àÎ1ÏX¿ãmt‡¼Lw¿áöE"㟿íËaè¨KAGNbcu?ïy—K
ÀM?–A¾Û$?Í(Ì®Ã?–,ÒQ?LÐG
ë—?BQêN!¡?îà^LfŠù?Ÿp¸{'Y?'B-ÇÅn7?‰ª'YA6l?'²­!™?še½·°?속Uòš?§öÛvÛ??´ÜŽ>è5C?£_^õ¼?›¼Lþ¯?ŒK/Û
M?íýaT%=Ÿ?œ'ë9]?œÙÏ/
ñ?äà;ã?¡½[Ò¥#?–È[§ZGU?ï´î/"8E?"jɾ¢­?Ã0'ü?ú?"7?rÞ¼?@9ÙüœY?3ôÿmn?¨ˆ†?'LPf"å?€@ߟ´z?qxÙƈw¢?{4*/M¨Y?~uÙ1EX‹?îIf6¦ìO?—‹-d
ó?¤G‡R??"]·ªÌ}å?ŒˆU—Gñ?í…~?ïP0"ªS?ntÊÓ³|?yhg@­¤?tûõÎàž?|õW+[‰?v‰˜\e+2AGN3FGL J0939.9-2831@p;vm
J@1Ý!ŸŒø¡À9s£Ô…þ²À;¥7†
¢¿¼gù訏E@…®	Ïã@Åt®¶â¿è_ä°Ëö¿ãe€ûñ†¿äÞn´ò¿ïÿ¤vЎAGNbcu?ïöL‹@]?QJÓ+ïC±?Jd8é{Ú?MŒEÌ?6µ+1³Ç?4nšŸSKÅ?ïw,BWÝ?'[ÂB?w1Ùþp?tÛðzR·?†tV{þ!Z?l|Õr÷?î'ü8(?š$ê±ic?¦Ig¯ÀC?–†
aº9?'œÑ"*i?€'ÚY?ïWS@]¾?ŠDp©R¢¤?s³aiÅø
?u0Q¡Ð?(¿Ÿ=O?†ºjÍèÑ?ïú(-Vá?Bã7Âø·?@Õ`©É©h?A(
ä…ÅË?#×üŠcs}?§péŸ7½?ï˟ùZ"?yý»Ûw…T?d–ú÷0?]E´µæÑ?oÉòƒð?vK"Ô—?îõq€9ºü?'®ïT'?˜›Ù³ç®?Šs‡/`u?'|hH O¶?rgIô?ïß×¢O	?d©œéQµ!?N¼Ï"Ø?Ÿ?C³@ÍÞd"?hy)üAžJ?cŸ¶ÆPˆæAGN3FGL J0940.7-6102@qGÿÞrÀW MRnÀ9ƒúNw\À;]¯"­¡Ž?ïÄ*×]ä@~ëÑL@^d¿9a¿Ód5Ë$<\¿ãÔ/5]ì¿ê"'ƒöo¿êb-à@¥•AGNbcu?×
£Ñš«¬?ÊÊ9v»•?ãzFö'!?ËIÓøSýó?fzƒ'?•RÐ?D¤Ð?Ø"¹gYf?Ñ>Fží7ô?ȂZu~Ì?½¬åô?ۜ•l'4?ËìkÈï:?å ãò¦?´‰ht¹³?ÎŒjjë?²ÏKE7g?¶Ê&Ÿéú?›	¡ø	|Ü?ß~ÐhkVï?²/«TD4i?җ?Gú¦¶?¶
Þ¶qP+?ËÓàŸ4·?®µ
í˜84?䧶W6êð?̸2U×g?Ճ‡?`#g?̑ÄK|ˆÅ?'ÐÁ# k…?‹•[ùÖ?äúDÂQÉ¡?Ð;iM š)?½?2<_¤"?¶3Œ¡…îŽ?ÍwS؉j?LJ_vF?ë¼jk^?§ªØçOi|?¸ýÎW;{+?£¼¯<£\?¢=¼Ÿ¿3Ã?ŽÌÆ¿-4?è(Óùap?¡ò–°½ö?ÄË=`]¸Ã?Ÿ[$`Áé?µ"åwÝiû?"Hã4†+MIXED3FGL J0940.9-1337@okÿÚ@@<g®¿›‹âÀ9«Væ—À;±gž?ÙыÇ㝸@V¹"
ä`@EÜѹ¿áÙú£°Úå¿åû¬'œ¿è'º+×Á•¿àf>"z~KAGNfsrq?ïóø-?`'"'ÊG?@H'¬gå(?@œ 02Lp?Q»²Ì…$#?^üâO|%?ï­Ð.šáÝ?‰eU¾O:ä?rSsâQK©?ƒ$¬–Ü?vÄtñ:³?{ É[£ž¼?î@,þ'ä?Ÿõ¶¼D]`?…Á9D?{8¾>gåZ?¦·ÏPêç?Ÿ nI.©(?ïÖ³Ÿ,3?r§®Á²/?9ÒyXŠFr?@>f7ÚqW?s	Mˆ«T?rVhÏo¼î?ïû¨Ën[†?JfZìÇ¡‡?*¥±*×%®?/ 3%tø
?5f˲sQb?GÝØM?ïâò4ª?hK¤ä~'?Y?…Ð.Ä?Up»'×|€?aNJ¤³¿?aiY&Œ,±?ï6S?õcgù†?{åü!7Øë?{ìlG}
?'<OÔ(·?Žò<¤ÊE?ïùÀð9}>?IËRäVÆ? ߝ:ª?µ7
´:ï?DÄX* ?G¢¨Qn?ªAGN3FGL J0941.6+2727@i$(?NÊh@H
÷Ÿß-øÀ:!>ºOò‡À;øgÕÒ/¿ëŠÝœ±Y²@
í1™*^@õíHû¿æzv×ÞßÛ¿æÆ(»,‰¿å'¬í€Ã׿çÔ`hå5"AGNfsrq?ïæêÍ5IÛ?dbb=¿U¤?M_ÎÝ?H¨'¾ž?aÐÁà{?a-—µ?ïsK² ?"q¬»km»?€¶pnÄÛ?‡	¡¢_b?'"ü«™É?ˆ0•î&@?î:wm¨W«?'ª†ü³ð2?"+|ü!·?€òiE=?¢Bʦ"
u?‹Ò²ûüvo?îð¯XÙÇ?"Þl;ù'?ݙ,-:?yâƒ6šà?™ò®›¤ÚÂ?'•p*"–?ï÷SA#>|?I¼».μ?9:ߙ?3Šï™,/!?F,Þtb¯Ø?D +9"ZÙ?ïՎV3W4?r"ÊâŽÃc?cI,ãª?bb^*<?fá` Þ@??i;.'Qq?ïL¦ï]?}UhmâÔ?ƒR-1W	(?q†pxŠ>¬?‰"ì{?sÄēãå'?ïÖ	©npB?jcÇ×?QÀ‹½:l?H/üBa–Å?p‹yy¨2?h™Êr#»ËAGN3FGL J0942.1-0756@nnY!…Æ@@(àaÕÀ:D"ÐÜýÀ;×Ê0:Zo?î¢Ðƒ6@ʂٹš@@‡}?pÙ1?ïþª'[c©¿Ø9î'N¿äÍExZ.˿䪀;ú'AGNbll?ïö￯ǝ?a$P'á
?(G ¦ìõ?*Ï6Flö
?N/¯>ëz?`/Z6?"Þ8?y;™øÓÖ?z}–C!â"?y]ì{["?¬)Qz¡?‹³ÕùÔê>?î˜%ž¨ª·?˜¾eÚ9?•RJn›æ'?‹ñbó1'?—©¾‡?'h…z}ʆ?îêáhÇ?œArêlë?‹ƒC%]v?"îß;ý@º?"ýc6"âa?—QÎN¹ß?ïýŸ'f€y?IfŠM°ö?"˜ûöÛa?
ãA ýS–?-½Kj?I/'·Fü«?ïÔ?Õ$Œ?r`ŸRK—?bó.…ÙY1?\9E<ׁ?hÌüb²¿?m'"÷M:?ï	lì"Ÿ?"j¹åÇù?‹ß"	BÛ?‡t¢?â˜ýA¨¥?~euJå?ï½£êÞä/?wÑwhü ?rò¥<H?cÒAƒ"ò?lvË)ب?r:zÂÄVKAGN3FGL J0945.9+5756@c"`RP/@F¶¬@eJÝÀ9§#Pg ¡À;þEE"n¿ã3ÿ‹æÔ@–K Kz@£	ÛØ¿å_Ð˒˜§¿á·ڌÿ俋8áP›¿ç>eðŽŒºAGNbll?ïïVJÜÀ?Y"gåÀ¯J?U"Xσ?Tæ=¸z‹ß?Il¤¸Í>|?Dë†Bûã#?ï†öFm͎?‰rLp"	?{æڑœÐ$?u÷q1UÃ?€OæÞ|?" ¡f:É4?ïAI,Þt.?›Ž'Ý?'ø´€?sìL°7ã?ŒµсÕg?w¿jŽþ±?ïUZ''{Æ?ÔynŸÓ—?xqáÙù)þ?u¶¿`"ãƒ?Žpnm••?ŠñÈ)?ïúWÜÛt?A&8P-'?9º	¤ö«ê?6Á䍝Þ?3‰""?1Çýe­7`?ïÙÌO#~µ?l•`]cŒ…?`ïŽ+
ä?UêB''š??eD"Þà?fKο|w?ï¯Æ|Ú#Ö?hB=™hôB?qÎÖ²ì¶S?\7YSõrÎ?vMêõNò'?_Š÷;G–"?ïèi'Y£#?bU·»B^¾?G°àAñ\??(¦²z?aªiEûs?aã6õû9AGN3FGL J0946.2+0103@mlÀ
¡©@CHEßÞ!‰À:•Rh' YÀ;¹Ã›Ë£?ã¤aöÑ>@ëréV›B?ûÏ¡‰Å?ïù«±~Æ¿ïþ±²{N?ïñ´Ï;MD?Ä ¾seàAGNbll?ïééø)?iIþ|jî?5¥¤H¦-?94uśÅÒ?caSY$Ó¯?hjŸ½Á]U?ﷇ­Ö3ö?€i÷®5| ?mÛ=é{Ô?n%»$¯?uNŠzãc!?wrØÓ«å'?î>ªÎÜWÀ?"øèÅ·ëÐ?Œ\k=4?­":×S?¥{÷sô¬?"EµP`=ù?ï%šT·?­¡ŸÌ‰g?MÄÀ5#8?o"üëêD?žm&ºx
7?­‡oZÚÛ?ïö3Ÿ%?T*+"ÞÂ?'º¡ï•"ƒ?,紘Îú?P¡mí©I?SmðZZéT?ïâFNÌtk?pŽ´Û‹ÎÍ?Y]¶;&Kã?W7˜íª?a
Ö#¶ß?h²öÍ}R
?îå2§Ðœ™?'°&í¸QV?}l³"à?qù©R2ø‡?›þ~áW±?'ó@JÜÙ?ïÞ+>´?wÎ~ä¼7?@nIŽ†B?P‡4ïû?ò?m­eË®6+?uà9
'<AGN3FGL J0946.5+1017@lïàÎ'@Eµ'ÿùJÀ8­@)»»-À;€¿®Y?ó|
‡ÃXZ@	‡±d¼m@©Ç`&[^¿â¸Œ4<"¿çÑëë1M¿è£:µ¼¦¿ç¥ÞvdÙAGNfsrq?ïøBxdY‹?H	s_¤>??"Lk&?=jóKÜVŒ?>Xð"^,"?;Ã*iI"?ïd(¤õÿ\?'Šã"û¯j?'÷È}Ϗþ?c,'?ƒþO¯XÞ?‹A`ÏKø¿?ï4‹Æ¥?‡G"V™ó9?"°ñ^ƒlQ?xPãßm?Ž,J¯ÓL+?®¸C¹¢R?íÌQÉ<?¥ËàaÖ¿? ÅàT¬B?"_=ÿÊ8?¢r*™?¡ö½»A?ïýñß?-"÷dPÍ5?,܃/ì?$JÂÊ0í;?!´\R÷½Y?ëÊ¨Œ?ïÁ|•/…1?vèN$$žW?oûI©kš•?j–´3?nˆ!-îl?q+À3Ži?>sŒ?vmÁbÚ‡?V¸ëµð?jý4‡'Ï/?€"ˆ–Œ&?lRÙ{†?ïl¢'D³?"h‹´È'?‡üë	bz?sógã3'?y¶ãb*¹‡?~™©E!]AGN3FGL J0947.1-2542@p.W /µÐ@5¯ãˆÀ9sHÌølÀ;ø˜,²?Ù¯ËàÏ»@$ko9Ê?ÿ30ßEö.¿Óø«oQi¿ß6N.í%¿ÝV=Fåö¿à겆$œÂAGNbcu?ïéµåõÓ?a'#
¸-»?[Úm¡`Ÿ?Yëçvəg?P¹Èëñ)?P{§ƒ?ï2:*Pê?¡÷–møÓ|?…éÅzßQ?Š'SL?‡¯ñ¦Ÿ1?œQŒSy¾w?ï%^ì
¦?†6m$p¢ª?ˆŒE{½Ä$?}ƒ¬ÁY?Žÿtp¾z?|–3ºjë?ìÈCªh¢?›)ó]I ?'"UϾ?†Ø£ŸËō?µ¾ÙmdÊ?™z©[±ì?ïù<ïq?C†Ì½Ìý?@Éë6?=iÊîB…%?7
‰r²€»?1Æe£$g?ï¯u'°Ê?‹uýüþ?w?pZÝ'&
?mT`gdaU?wêYðÍ5:?…þX¦ƒc­?ï"îgYÞ÷?r܄%ð#Ç?{'帤?l½'k¥v?zq9vîǽ?aü	wŒLT?ïC{Õ¹Z?ì¹ðZÕ;?"ï~JãÈ?gȅÄhbà?•KJÌÅ?{}…àvAGN3FGL J0948.6+4041@fžP >cé@I+ŸÀûÀ9é ªšrÝÀ;ü	Iú¿ü¬iøÂ@ʚ‡«/™@Yÿ¿"S¿çþ€!‰£¾¿çVŒ@낚¿æINa7…¿ïÿñ([AGNfsrq?ï¹yHkS¶?‹Ú!öª(Î?Z®Ð1a?eÁO>ÏB!?|—§¼ž¶?ŠIJ'ˆ?ïŸ@;s7t?ƒÙí)ã ?vnÞ|oÄ?tòAÓ<±?yñ¸Ç1W?|•™¨Ð?í7"Ýäþ?¥EÜò΂ô?¤%GïûŽ?ši¶Å&ú»?¨bj4Oˆ–?¡Øõ–màÆ?ïœÈ±›T@?ƒÛç€š?dh?ÏaÉ<?q?Îl+R?ƒ³Ã›³•½?&²[y?ïÞ»Êúm?ŽôÛG]?fÍ Yd¿?x12\['?s(»rø¿?‰S›$âw)?ïÝ|Í¼?s¡€)?aŠ"½«Ã?pRÚÞ%&?`øÝôªÈÔ?a¡Ž çƖ?íÛw—]¡"?¡…#±µð?£ñqÌêâ‰?›æØ·rº¶?œ®)|-ֆ?—.š­½K?ïòû£ás?Zd0}_Ÿø?Oàæžù?%ñ	Øh$
?XrήÃ/?YۍÞ9+§AGN3FGL J0948.8+0021@m'Þß)@CXßÿ¯x(À7»¯ºmÀ;Y	Ó¾X–@Ü^žà@V©¡#¦£@é‹+홡¿ãøN§;¿é/2°ßäà¿ê"9Æ^•¿ïÿ
1ŸgíAGNNLSY1?ï£û
Ù?†úÊ?…/ÇúÈ6$?†žþ(&Ÿ-?M$队·?H×òa³+˜?ïOŸ"I<? ÓºÍè7?'EÛ4!M`?™š"K	ÛÏ?ŠàaÀi†?Ž¥—Êb¦?괐÷š¼ë?®¡ÇL›":?À%¡,éu®?ªQ—gR?¤ kÐ¥—?œ›ÊRGk<?î0¨iÁæ?ªÒ"˜£}Þ?£[Lj≚?¦ÃwZظ?"3p'º~?™k¢• ?ïŕè×fÑ?‹8ÖIóö?zy¶ç;š¬?Š¾¨+^¦Ê?EÚ¦&2UP?D½ll^±?ï[WƒA
?¤#^ilÖ?…ï,sÊ?ŠÕ-†k­?ƒLšôÊÿ?6jèY°?èú՘<;3?²QGEcâS?Å%̉ABý?°ˆNÐj?«»tPXà? áh±·v
?ï~ÚnBu?‡!tïÁ?Š!‰@β?ƒ2šY¤‹a?i_P`¸K?v›ÜérCmAGN3FGL J0950.1+4554@e›ú€Ïž8@HÜRÿ" À9ù8¶Ç¨À;Õ
¥uoï?Û´þ,žÍ@‰}dBö?ÿ3˜Ì•¿êøÖçU‡¿ÖT©dÊD¿áf¡³¯õ¿Ï'·ïdAGNbll?ïëšmTX?r°?µ7ð?HŸêŸ?Zû¸µ£n?\Ë#fÊ?j$3`©0?ï|@ "&?V¬Õ£š€?~âݒ
Oq?'°'¿ä?~iö¿h¤?†JÒ¤6²m?î·½ñè"?"1Āõt;?…Õ&itƒx?xû)üÚ?ž®ŠÄ?'ÛÅÏ\½ÿ?îÇý2xÖ´?–=ÿ¹
Ÿ?ˆ…,NR?ø<§úP?š½ÃczJ_?'þ&Õåw?ïØ/âç¸?¯S­èâI?SÕýAƉ;?Ž2Ihσ?må['[c?§È'kØ	O?ïÕô`ºî?tŽ3éž?d@=ä8b–?jœf5e©?eËaKJ/g?ho©~9§?ïtÈ&v?G+¬ŽæN?w½˜]΢?eÈA'9…Š?†ï2bAÀ?|¶gæ-Bò?ïºìð%8ì?qÙ:À"Ã?pƒÈ²môM?c[-©U¬3?r¿(g±Ï?hE½Qï1AGN3FGL J0953.0-0839@nř'ÿ@@óàVÀ8H.Z†^SÀ:ÙFóÚWÐ?ñ|Çô ÑF@Úú7äž?üâÝø]Ê¿ÊQʑÍâ¿Õ»ÙÂK¿ÞŽcMµÉ¿ÖtËí¿ÈAGNbll?ïöyï҃?TžaÔ­M?>ñ¯¢	c?IA¾ƒ.ž?H…?ӏÑ*?GO|֊í?ï"kM¤ó?ŒF	ä*B'?wÿ"m¸n·?w²}wAXz?~JÆ
õæ?‡f'½#ºÚ?î5'3ݎL?œ)dH)?–Æè"Dr?™Ö_°…=?¡Dh{Ãÿ?•œ<|ss?ìþo1ĦÁ?¢BÖ-7Šu?…
ÂíB;£?ƒÆ@yÁZ?µjÎz´…?¡×ù­~Éw?ïüIyh:?7Î	§j7Â?-K–c6FM?1¦þµ¥œ?.՟–u-?'ÕKU‹V?ïÑmZ˜Ê?wïÅÌ-º«?daÐ?˜?c:)Ôû?jÂ–è;?råF¦ôF?îú…º"K?'Ñx
Ü?#4TË?†Í8íV´?‹Ýö7Ø?‡bÞoØ=?îæê_¯½ó?…>v†¿?H!3Û¿y?n‹Ñ¶Ï?š~£i¿ä?ƒ®"½ŽAGN3FGL J0953.1-7657c@rV@ €À1‡@zC"À9ï›Á''À;ü#Òm ¿à͙—Úìd@ÛXè#•[?þ—‡€½Tµ?î"NX&C¿ÊüýRaÞ¿ØaiTµík¿â¯š
hõÉAGNbcu ?ﻤ{n#?{z6m8^?QªÞìÜ  ?Nÿë¦§â?}Ã
—庱?ysì0Vé?îCË%²'?µ²Š‡?ŠD}'0?˜à+çI?¥2LÎý¹?²î5™
Þ?î>QÁ¶¾?"ñF鄥?'*/ølî?~'©û8ˆn?£N̢ͣ?Ž1°Vhz9?ëµdBl-?ªL©2C?ˆîBc2òt?ƒ©^·U?¿7¢ËéÅ?©*Ch"?ï瀦ÈE?c%k¾LÓÚ?;ìxÈ @z?;0`âMã?eÊEŒ
Ù?a'ö]MÄ?ï|^-eq|?™P¹o¼•6?q`ºS›,?u±WÁ'1?ˆ8q×Jå?•¾-¤Ä?ïRèã-â;?z
'~-Û?V¬!ð	?gŸúßJ_?Š(p'65"?rßù´¾6}? _—¦?Šºâh¯Ý?kjƒì)ó?]ñ²'Š×?¢¡M½Ú÷?‰¶&ÛŸ<AGN3FGL J0954.2+4913@dôªà~Zy@HÉö`D
vÀ:©î,˜å?À;Ë¢1Ð?äL´Ø©Í@°†'¡Ú†?õM9§š¹?îwÂ%Ì:¿ã¤ähŸÑ—¿ïÂ0œÞ{)?ﰋ֍jâAGNbll?îÑ64ֈ?´6üîíM?_¾ À€õ?mÔ½p´)/?¡ñ+•žÒ?³úˆ½kjc?ﳀã;ú?ˆî¨|¦è¹?qR{w˜†€?ƒ&ÞPÇq?tíz)T~?y¶è*¿zã?ìaýÒîœ?¥Ú'€á,?°øhó8»@?¢*hÓ5ï?§ï]Nm¸?™jž[)¯A?îãÁe2P?§ÿKVîãÉ?vXº}Ö?"à5O¸(?ž}2۟y?¦€x½)ae?í߀׌*?Æ,ÞvSªˆ?MÅ\¸p»Ž?_Fw§7,3?°Èu(Úî?Æ.0ŸtF?ïæÃ,~ÒÞ?e÷ý21_?W'¬ÚMš¼?V§Ä¤©t?[Qú*?\²[ñ91?í¾§è^E?¤Ç˜úE(?­ƒ‡Ãà? èNÕÈka?¡gýpÏ?"qX¡›Šy?ïà­
Ô^*?~".jM?DâÞÍ¿Ð!?q)֖æ¾?j=€Ú?v¾–¸B™AGN3FGL J0955.4+6940@a®+ÀãŠ~@DE…`&±EÀ9A¢e6À;Ï"כ\è?Ñ9Ô
x@
xjRWù@®#ÿ¹‰#¿ßßëÄ¿ÞTžç·4¿çÑ,ÎDœ¿ÛÄę!¥OTHERsbg?ïWîî¶?‹I•"Ñ?…IÁºÖóE?ˆ#óزç§?jÞCò
?hÇ»ÆX?îfL=½?¹[‡fñc¡?¡ÙÑ
QÆ$?µÍCtôɖ?(ÇI€'?¥{[O?ìÙ˶ªÕ	?¡¨½?¨{(¢-n?–º-'G`s?©èõ¹\?–3Zœïê}?ê…
ã«-?º8»»àôÖ?»Ï›b‹TK?µîZÊ}œ?³¼<FÅEÌ?¬'å/þ¤?ïÜAÄña,?oÄP€?húIl6ˆH?im•x{~?U‡ã9ÑØ?U¹5q ã?ï+~!ݺ?˜m;[Œ"?}äí´‡´O?'y
Ž›?s…SMRˆ?…ó¥\N:?î´ít¯vÈ?€%)ZAj?—k*J E?‰¡ƒšj)3?'÷'¹?€ßPYö
?îõ.æA?'bSaoêE?'/¥þåuQ?"Ù÷3Nö?ŽU.¾Uüç?ŠDNŸ±qäAGN3FGL J0955.6-6148@q»-ÿ'+¿ÀÈÙà0¬ÆÀ9…¦ a4À;dM\‰?êÄG©³@
}~
@›_¿®+L¿å÷ó4Ѫ¿â·K:Þ¿ÛY6ÿ⺿îÏ
L½¦rPSRpsr?ÝTŸý¿f?ƛ½ÖdÑ?ÔjÌMñŒ?Ä<ßi1?́'ßåOÈ?ÁqNÄ*´?½'scµ•?À*­
ü?ÙLÛf~ËH?ÃIç%úï?ßNÇ¿­æ"?ÅDQY*q?åoÎ]½ ?°ÃÝkf¼‰?É(€¡Œ=?«ÉhéHd?Á´eçD?£ ´ò¹¼?àؖ
²¥H?¸—4z¤Z?Ìà|"4¶Ò?º^OÚLÆ?Ͻ+B´?±Eh~S?æÎ?R8¶?ƒm)Æo]?Ç©Ï/0L×?½£X¿dý?º:gI#œ?³;Ý:r?ÒTùğ?Ȋ¸Y'l?ÖËæ3ŒZ¨?ÂD:H˜¡?Öà
ÓSà¹?Ã
Ã÷ÕÓË?ë7ˆ¼ko?¥géq"Ù ?¸ÅSíÏ(? Ú+ßEº
?ªüÌa‹Â?'/€j+?æɬI¨I?«‰^±Oê?Èe>!L4?¨ôx5"É?¸è!}ÆWÒ?šh6Ð?«¹MIXED3FGL J0956.6+2515@i¯?p]@Iwù jn3À9!Áû¸r£À;²#ÃS§G?ðÐój›TZ@ÒPw¹Ë@|G '¨;¿ãGXÕ6Ü>¿äãëSdoÛ¿è_EüŸ´w¿ïÿ˜µÁ²AGNfsrq@?ï⇑%Ï?kÊYmÃ?gÚ¹»HN!?gžGóÆv?FvÔ±'½Ò?SŤêщ¼?ï7ÓÜ¿Õ?"ÇÜú¡¯?‰—IE3ßØ?‡ÇQµ?'?ˆs¿'ç"Ø?Šf8HdÖk?í_Ú#ޒ®? ‹EŽ——h?¯
À²¿Õ?œÄèm`Wc?•ï:ˆ:—?‡'./ƒÊ?î@'Æ»³? W†°¥þ?¡¿s=§då?™(NÂå?"pÀ°ªod?•7h—±?ïì"ÖïÃû?d¼ššápZ?`SÙ¡³I?b˜:þ¿rK?8ºâ–_a?D%jØn÷?ﬥç'8?{½àaÞN ?v¨rÙFã?oۑj‹$?sNº@4ÐÑ?qåþ=Zmþ?h¿Ï?""¾\Yh?Ÿý^øÏXD?ÞÛ$ûÎ?Š¨#Ü?}'«ÿñ¾ÿ?öì?{÷'«ŽB´?ƒO«#XÄm?r7@DNõ˜?m9]"é°*?r\P¨VþAAGN3FGL J0956.7-6441@qك @ÀÀ'{ 4hgÀ9´Ïú~¶¿À;}hq¡›¿Ó>ehIÀ@wZ!‰'@Ià [R¿å•‹g>§¿é‹åô¿å	=Éí¨¿Ó=X™&àAGNbcu?ï•õVú?ÿ&S`V*?Z€Alªž?ZÒùØ5Æ?‡2¢Z+œE?Žö+•Úó+?í͇~€?´jqýéè?ˆWP¶á/?"L§t?­cc§š8?±`ʓ^,‹?íìՖJÚ?–"qA(˜?—1ßÓo?"qgÕ1	_?¥™·Nt¡?¢DBbÃ?îGmï¿'?–ßé¬o­?]•dðp?_IâäG²?ª TUº.?–´/7Ÿ*]?ïßÈcËER?t+§dd®Ø?E¶ÎF4?DJzï\ú?j÷~˜ê?s<áÚ;zs?ï?ãP‹¢?£QlXh­Ü?s]i'=ÎM?Ì`W¹é?"F)+³½%?žîE;™??ïRå@>½?x
Þë/Pâ?Á:´
8¥?kðy2•£?‰…u+mo"?pï&.Œ?ï§'-/Qì?q‡Š†×Ï"?CRÝ/h?8Ín²E¸?…B«_å?q<$gv-oAGN3FGL J0957.4+4728@eA¿p@IIí )k3À:¨(÷À<ÿ™¨³?åðQòċ¾@"y$én@[œ@gú¿Ùftlþ¿éÅÿýËÑ¿ïj'"?ÐÅ@CŠµAGNfsrq?ïûEmÁ­?Fp¦°úq?7ì虖*?>|ßdè?+Ö(æͺ?50 Õz‡™?ï¬V+Ÿ"Ú?ˆžˆ%''?sÙ¯L,_?yFs~À5ù?uû;ââÄ?~º¹bÙ\\?î60Ó~å?›eƒ`|?Ÿ
ä_´5?–vl?"ªh?š,,ÿ&6?mvî!p?ï'M€—a?"°SÌ.7?s'¨"ùìª?†ßu‡EÎ?…ØæäsC?V†®â)v?ïõwËéwþ?ˆ™ G
´?IõfM^"?'é]º
÷W?@ Û¤Kd[?lÍâûà?ïâhZ²S?p#ۃG=n?^6McL?bͪ÷¼g?]É,±G'?aŒ7*–†?ï÷öú¦W?'j©^®?'•°þP'˜?ŽÈîŸD#R?ŠÖ =Ö,û?'ïc'âÅ?ïïsðŠ
­?r"`‹VC?GeLýÚ?[0dNñ™"?Ue°Èns?oQ-‡1>AGN3FGL J0957.5-1351@os Æ´…@?.²˜¬4À9_ÄM¢JBÀ;ªFX©åA?öfàý0lÚ@wŸäŒ\@)=³ê¨«¿ás؉ÚP¿æY<Ž&¿ë8ÙP;y¿ïÿ"û&ýEAGNfsrq?ïË{õ!ˆD?v{r/$?u²ióÊ?t©™a¨v?R>q %—?Q	$:½?ïDPÅü_H?"ì±€?‡¾ÔåÀ¦³?‡ÎÔLÀD?‡,ù¢¿Q?Œù«·…;3?ìsêaf?£ó¥™K"æ?´`ÚyGdz? 6ña]'? ê
R²?'Zu"9Š?ît-zŒŽ? –ZïÁ—°?Ÿ'ŠªÀæ?™çcËQ§?'ÛÏ Æò^?'Êôr' ?ïäq$–žy?f} i?gæÖSØF?e¸º–a?=@)AÒ¢Ô?9_y`f–n?ï­zGÕè»?~åÌøìb?u$OµˆÚ"?pMî)!º ?tŒLDø;?uê®íY?í¹¯|ëõ?3*ŽnÏ3?«•&uÆ?™‡6ââ…=?'ŸÃMsۂ?ƒ¶ƒ§`k?"mk?ñ‰´»Z?†S"âRp?v}ö_ìÇ?i¦-¤ìx?qŽ79ÌÛ3AGN3FGL J0957.6+5523@cÒó@ÔÜf@GöãàÈñÀ7nû`^À: u'ÊI?øÂjž.@
ûãL@€?ýÌðW@"¿ÙNKÏié¿àšÈ0ŽpÏ¿àÕ£Ñçúâ¿âd»rv-óAGNfsrq?ã©·Âà û?Ã*ìы4?Ǒ6倉?»ý "µ"1?ÉÇêüó?¾?Çk9	?¿æbú:'?Ç[Ÿc6U?èԃÙz?ʓBó½–?¹u~8=~Ô?½½¿ØaoJ?ã"ÅzP±§?³}þêár½?ÃßßêòãÉ?©o€ÔAYh?Î
+ÊUœ?°ÐÖä×?±Àn–Fäý?¦K,X‹?ã(R/€T?ÁO¨QöËW?Õ?·¶F?¿å€ýfÜ?è	¡B@¨x?Àù³ú\Á¼?¿ähèÕI§?²ßFGÉ(?¿Î	põ"?¸³ƒ¯rTù?ņ#J©ƒ?ÄÆç±jœ?çkE–À©Ü?Ȫś«Å?¹™ŒHAE?º^/à/?æzàC2?±‡!Tµû?ÁÃ]Ò
)?¦¢Ø¹ha«?Åò¶­óæ?ª³‹Ð[·1?¾¦IL?£]ÃiF¡—?ãC'OH<°?µGšùd?ÑÔ³Ï-'Î?²åˆ]ñžMIXED3FGL J0958.3-0318@nD¸€®@C.^è¬À:uÓ|ê6jÀ;—ÛBö?ç±Ä‹_Å
@
wã'_c?ø=ÖÀ¯?¿éśžæ¿´Á¨Æ!%Ù?Õ<OÞÜç?º¹U2AGNbll?ïîR(ÊW/?båJÝ÷Õ??G÷È<ª,?;B4§"?[‰°$˜ä/?aX†ä"o?ï²z¹Y¨h?Ü'¬(}?qœP‡DÀï?wI¼2‡þó?u&RÄWç'?uVÞ¶¿§C?îÍäƒä?<Ïn؎?Šg-0›Æs?~ò;Bâ'à?™ÙÖj3?ŠO°Ê>?ïgØÊd›>?–óÆYí¼n?Oô¼òù?cǁOFn?'ï<—?–Ì?ŽTNÞ?ïð´W­]h?c[€Ç¢(Ò?3F¨ù»o¼?-FL¢"f?YŦ¡D2?cŠá=o¿?ïä;Kä¸?gš*•­4W?WÃö_¦We?SÊ$n!ÛB?_ÅrK³?aíÏôn¯?ï.ÆPÿq?ŽÃÊ«Æ~?'1u;\H?}Ÿ‹ð|?'¨¬Šv·?Š@S‰XŠ?ïØÏïŽe*?q—ÑT³A?Y_Œa0Ÿ@?a;ׇ"ð&?j€JRà}Ô?l)N!¾AGN3FGL J0958.4-6752@qû™€o&)À$Š>ž¡@WÀ9ûͅYqÀ; ô‰u?Й¼(ÃK@
áJòA¦i@§ø`ygu¿ëK"ÞK¥E¿à`–!ƒÍ¿ØP¿ˆõ?¿ãf"Ú ¨ŠAGNbcu?îªÙÓ™´?«–&§ÇuC?koÿgŒÕ´?m©ZSËë?£›bÖËã?ª;[в?ì{+¦2??º ozûã€?–•— RíÏ?—È!O,¤?¶<ç£#?¶t)RÌ»?íÈl•bd?šç‹‡5¨~?—*¶?"»+¥ûE¿?§ä8"I¿?"Ùx®qÕÌ?í^á{Ü?›yÛ$|?†°‹ÎÕM?nÒ¼À?²2â­ïú?™ä*Òá?ïl.·´ž?¯îžESè?uM}Û¨~?­Ì¾©ÜMl?ŠU2ä´C?–Xkß
?î¸Í»×~y?¦ÀÆM9–:?'ÿñ((›?…þF ލc?ŸfOë$ќ?¢¤±vkRp?ïM,c`Lœ?|¨"þd'}?óDe¡¤?p@ [Ž?ŠÁÒìÎ)V?s¿×\?ï7awƒ!?}!(³lBb?~û
œ‡Ÿñ?fk'úڝä?'U
 à?w±þː¢AGN3FGL J0958.6+6534@b82€ñ,(@E&Ÿ¦ùÔÀ8¾­µ°P•À;ÁUÊ6ðW¿øv†PÀb@ÃÖDDÓo@
@?‹0J¿ã•Ó€ná¿åÒÙõ‡à¿ä-Í÷!é¿æ®ƒZµO¥AGNbll?ïýˆ}¬B?(¡~àU[\?
uæM?	D–oí?-íA'õ?%ådsjN¬?ï¶"ÅcH?ˆ¿á8;?p¿#D¿T?'t˜J:"?tÙÞ/W$å?xÂIÞ%J?ï^×D†(	?z'žÓܵÊ?xº³>Œ$â?aã Ë³c?‹ìÕA?¯P?v9Ž°=ÿ?ïòÌ¥Šz?b¢Áoø?]'UÖw?%~åü
?YÔì'D`W?aë']¨}¾?ïþã"ôÐ2?gÌËL?yÞõÂb?ћ)©³?"Ë"If#?×Õ䇀"?ïæ¤ÑIøá?h:h5"J?V½~¼ ¿­?UßqQh]Ñ?[øß9]Ý?`õøG€nd?ï±"lj•?håö>×D?m¤hîî˜?Q«½"Šë
?xœ|²·ž?e?05Š¢ò?ïþ;~Ӓ?A@Ò7<`J>Æ7å‹6=>Ò©býDQë?+ïēǦÃ?A@)Ó;³¤AGN3FGL J0958.6-2447@pDêŽ:Á@7pæàtI~À:
ZÜÅhTÀ;Âá½Ùà?·3Q7Ágˆ@XÓÞå@ðp¿…¼m¿á\ï»Ü¿åºH싌™¿æ\wÜtNu¿ÔnRÍF3AGNbcu?ïéSx*½?dç/‡œÅ?VaA¶ž**?Z ™kãG?V€VL¬›?XÿéK\ñ…?ï~¹T±x?"x=r_¤?z‹š¼P?wOpœ{¬?ƒOäù¥,$?•U[#?îË@̧£?üù9b-?ÎV žç?}¤|²T¯?—°ÝRâî%?"ƒ†áÛª?î¬Vu,§Ô?" K ¦ö?wtyTÖü?xYKŸ"5?¢L	…õ(à?"-ÏñðGÑ?ïøúŽë¯€?W*Ú¬ƒá?<ÞòrZ?EÕ¥¶JæÁ?<)ª(?Tñ?N§…§IÀ?ïÕtï	?tSÊG®_º?b<šÎ?^žó*Ɔn?h‹à	ö¼ö?nÊ€ž$1?–´âË?w8‰™ÔJm?zn€¾ç¾ä?e¼FÁR>À?š™ä5%Ô?qèêpfç`?ï¾D@C3~?qƒ.…½ÜQ?[†$óŸ?R.(™ëÀ?yüV FA8?nå¹AzÀAGN3FGL J0959.7+2124@jtþKZ@IQ4 ½À:[®a§ºÅÀ;äEÞ0¢_¿þ‡†AM'P@Þä‡(¨Á@) CVí?Õ®ï1%¼Ó¿ß"ç†óŠã¿ë>ãp?›+á
ÈAGNbll?ïì/
¯†k?fW˜NW\?ZyÅOÀ1?c´Û+m?J(á#ñ.b?KbË×¾á?ï½¥+aòR?~Eîózw÷?l>h6?mß&'ôF'?shª	½'?uC§ÓÐÃn?íèfžùœ?¢¤ðagÔ?§ ûl*G?¡3îô¯Ú?"âê(Néø?ƒL°«‹›?ïÛ.©$•Ð?t€E2U¼ò?
f݋­\5?ô "b?r3Ý¢:?twý"J7L?ïø­`å?SŸ%½.j;?B,ÓÒEg?M'ŒtՕ?;(ìÀóí?='ŽHã?ïá+L¯?xЃ?^ UCº?uèÚÁYI?_‰ãÖì?c	‰Ñ°xb?îç;1ž!'?'¿µšÓ–Æ?—àe¯'™?f–Ò	»?†ph:)†1?v¦þZ3ø?ïû
(¡M²?D¶Hæõ>ÊûÕìúD>Ít¾,nÂ3?C°bµW_?D¬=VÓDAGN3FGL J1001.0+2913@hî^ß)@JK8_ÂÞ7À9'Ö!à$˜À;ÁCÂÍoŠ¿ô‡XC¸çh@ï1Æ̂¥@A›Ÿ®0ª¿á;™Užd¿æ›Siñ¿áhòüGŸã¿Ó—Ãl7AGNbll?ïþo<"ñ?ä"ûôû>ÿ˜†wÊÏ>ó›2â`?"5÷ú,Òé?ÙÌך?ïÄÚ¡»jé?}'F\…
?i
³4È?lÅ'3Å??q)ڎ;K?t":ñ×4?ï‹TÜ?i?wÆï~ý?sP»Ê†K?_~¯fÂ"@?ƒ'¼˜'.w?s;=¯Â1µ?ïùð—cØ?J7Y¦"Â>Ê)ìÈãˆï>Պû;àD?H#ybRäÙ?J0¿o÷Ÿ?ïÿ=›I¥™?Ü$ÇÆò>ýõ5°ËR«>ò—Ü&?ÏCm`«ô?1ÌþíKâ?ïêƒÕ?À"?cû¡þ@W÷?S'¿ôŠ?RÊaÊ_´?Wf– 2•u?Z™ÓåÀš­?ïÅF³:!?c"ºHr€í?g#ôçÌ/?MÎ~åQ?qÊ«çzO3?`þ»pÿ©?ïÿDþ%¤?Ú^ <R™>ªwœÃ] `>ª;þ³ÿ?+N3Ió8?Ƒr¤OeAGN3FGL J1002.3+2220@jPå`A‰7@I¿f€g™lÀ:d~¡ÆÀ;à\d"ä׿ǃ'Ù6Ã@ëþ<[{@x¬ßœˆ6¿Ý]ޞl£S¿ê8Šò¿Õ2–È%j•¿èB`é"]AGNbll?ï¨f|œïÌ?•»çáËîs?\÷ÕC#ÐD?c«}1-m?'Gf8ž£?•c–óäù?îôJ
P†¼?ž'>ç¤òò?'	-ü©&?"§ã‡™ÿÕ?ŽÛ"ƒ–*­?'Ï*
H?ìú;8üÿ?¢sŒü""?–äHz©O«?ˆ_-¡ž¬Æ?²u!q«?¡
Í>©âQ?í48þ˜¢?¡P³rnî†?•¼¾Ñ{L?þç¬@#?°ïZbn?œ× ¦ã×?ïëâð-W°?pÔ-q+×?:µS'HRO?<•ýìlU?`ÆegÖXˆ?py±ûšÕ?ï¿7ðԋ?|º–ù³ ?pêÊpÌ?pjö`z?o
ª`,å¸?q -_ô,C?î½ò]bŠ?'"P?…õEuÅ?|zs€£?_ÙÀŒ]Ø?Žåˆñ<?ïLK3ÉÊÔ?€,µ± u¡?ªFG/'?lAæ¥Ìõ?‹BìÃõÿ?xÎo¥,‡aAGN3FGL J1003.6+2608@i"&?šIÃ@JV<ã.À:nˆö´&äÀ;ãØ$ãý¿áYZŽ/ÇÞ@
ÃNÿl‡=@UÎ 3ý¿äÜ4~]z¿èñ*,××ö¿Ò'i!à-¿êŒ²$ÒÏAGNbcu?ÚS§?{B9‡÷_ç?fjTÍ®¿?eFº;µÇ?wkkì5(?täSà}‡Ù?ïopBÞ!?' þœ5}?ƒ´üÀA?Šü_îobM?:G@/Â?'ÄÇû9°?íŠu¾ŒÜâ?œJ¡,ø?¡W'Z‡•H?Œo˜ó¯?¦¿>Qœ?'ŒÓE^o?îÖe|?'`'çÓÌ6?uçÝše?t<´=CÅ?ŸÅÜ3?°Aÿ=?ïêY±k?`Nº ià?Pr-')1v?Kç‡XjA?ZÛµGEöò?W¥ûåÕò?ïÓÌÙ J?p†Z®ìvê?e4>©´±?aPh¹'@?fþèÄø1?e´)ö)¨?ï(g)?‰7U]¨È?ýêôLó?$µÒvc?ËJÑÖ?}/u×TŒ?ïÃ5Åg[b?jh&;`¾?`P;ŸšçÜ?QàCÜבŒ?v<ÿ~"ŸN?fƒš@•ìÆAGN3FGL J1005.0-4959@qYBà°«@
Ý¿ä1À9 –6—À;W¢Õ'}ô¿í¾¾Ë='Â@
çEgée@78¿å׿é殚T!¿èrWý(E€¿ç.ϧ%Pû¿ä"0™[ AGNbcu	?îÎàž÷ã?¡¹2EŠi?0wÍZ&?|/6*ʎ?žWÎ,¥"Ú?Ÿ*×h2ù?êð³[â?Ë9¸U˜
?—*qä6{?œ†Í`±Ë³?ÄÖîõÒ»µ?Ée5¨1?ëe3éf‹z?ªE¯KWxT?¤ñ9:I­?'u8@B>?º]Äîÿ¨?¥·™,2ú-?ìá
P3Ž?£ì¬óó?sœxu6?of¾1rΈ?·½Ëü8p?¢Í ¨É»µ?ﱏÊbå(?'™ e¹·Ù?d®œµ«¼"?f}3ýž~î?|à̎"Ë?~î'?`£ü?µñŸÀÕ;¿?}°ÜX¿_€?†XñŸ?¢Ïnm¿ø³?²ÕQìáß?î¯,µ.N?Ž½3ºˆË?7Sóğ?x¥Ü‹Å:C?š~¢§-ò?†×>Yê?ï6{¶7?IÀ|S*ÿ?QÒ:ÌæíD?DgxǼÿ?˜!ÚÀ>?€å]ÃѺÁAGN3FGL J1006.7+3453@g€Àð¸@K6îÍ©À:¾ž\vù\À;êň4íH¿×ך3{
@@
cJØkf€?ú|R@¿Ê¿ïÿ
ç\›?ïÍ"Ê5¿ÔÄ@ٱ뿹ܦ/eY‡AGNbll?ïù9Ï{ö?Ee±xq?/Ù*è¥?+ÀÄÖ°«?C"}5"³?AÑMr
'?ï¢^‹óá?…­–²Ó??vCô±û2¹?{jØq¶ÈŸ?xŒÅ7ç~Ó?},´ O{?ïY|"F1?¬t¶_öÔ?…e˜œTÆ?qðWTqd¦?'¢•Ë?y æõkô?ïp=(Ä3:?Œm#BE?~ˆ‹{ˆp?€ù{Õ¯«?"¬pv!:?"´£Þ??ïû¶3%ê?5d}ûš?#`Þ$؎a?ð\·¶(Å?8öÜíO?1]å¬Zã¡?ïà¿ã°>!?l‡Þ­'?]òO_±õ?_Ï8;‡7?`FôÙ¢Èh?aœpÅ*8-?ïÊ.s?péѸÂpR?z{á·9[?fƒî=‰/?'þ\Øñ7Ù?dþä*n4?ïãè'ñ¦î?]ìtk>'?X1Å>÷Ù3?Lä.Žkç§?_ý®ÿš?VˆªÿVAGN3FGL J1006.7-2159@p<۟˜·@:ȖÀ¡E`À8¹æè¹À;ŒÕÓËò?Åò´âd'Œ@.ÁКaÁ@z›@7Ӂ¿âJ°7S¿çæ `U¿è%=ÍÒŸ¿×Æ*g˜Ñ¯AGNfsrq?ïû~ä6 Ñ?6h3iÇs>?0ßÊæx±?/$P]åµ8?3jÿôÏ,?,)Äýþü}?ï¥8AÌr?‹"Ñ*?ô¬?sƒÄûœ­?'CIiÍ}?yà
n%?åq?ï/¸I)Œ
?†Xß4ñ]Ø?€J«ÛŸ¨C?oC˜e´´?'ã ïfd??ƒ‡ñ"8?ïUiȊa²?ø•Ì‡6þ?[ïÆ~)}´?]Ž@ëB±¾?""Ê~'!î?‰îM¾2?ïþ9\Ô'›?"?¼~Þ?K3±w1N?o*2‹D?‰* 8?ÑB¹F~F?ïáÕÑЏ?hf•¡—ˆÖ?Z¬Šì9oÿ?Rº½?¸êÿ?a'äú8‰?c4Å4-(?ÊQ¸?qڙJˆŸ)?sc¯¤w^?aó¸½ÙçS?|\" K™?mdӃ+¬?ïåùàðßë?i}3÷Ç)?9v¤¹õlÎ?/£É[CÁ£?f×J´([?h9Ef\CAGN3FGL J1007.4-3334@p¾%`A‰7@1é¬ "ÚÆÀ:Ž(LOdÀ;¥¹¯¹–?ñÃv¤÷ñ"@·T?@N[ÿ…0׿ßúú¾]Úb¿èÕìÅTw¿èq…­Ғ¿ïÿ8Ýl,NAGNfsrq?íGÀ<µVÓ?¶:/?·^?²¡þõ=2?µ9ïm"6?‰Ca£?†kM˜ôŠ?ã×S:±ú?ÇLßµ:h?ÑM€b!Cƒ?Ã.šÈÜ?¼d¡ë!Í?¹bnÓ%	-?æØfe‡Ì?²¼œ6@©Ÿ?Ç՚aü°{?­_/ýûl?¹'˜û*?¢»Û—M¶ƒ?ۀ¶Á)O?¸Rfñçé}?Ü›iÂ*K?¼Ö'û'Óì?Àõ[ªSXË?©ô…¶S\Ë?í 5[Ú¯?µ'‰â ÙÛ?±àbŒÚG?µ^÷˜c ?~ÇL;· ?|woût?ë¡c¬;¢?¹Z \òÃX?ºJÝϵú?°c›Š\?«/ªÀòõ?­á¼¡p"‰?ë]'ÝÈ?¥W<´³É?¹¹Cò·Ü¿?¡'ý?S?¦¼vÖZœ?'0sŸ>\?åãd-YÍ?ªr­9½­?Ñ3RãQÉv?©hZoRÂF?¨/'À0'?",J®~-MIXED3FGL J1007.8+0026@n?@OÂ@EFv¹ÃÀ:BôˆÓx¸À;Î))Äõh?×Íí"äg@²A±%@¶'¿t?ïýÙý¡¿å"­·]Ï¿¿×®O½Ç:+¿ç`n©š²bAGNbcu?ïí¶‡žð?YÚºxBÑ?Jÿ Çžýa?K5—NLt´?W(f0¢"?RÂÌ՛|?ìÿ;©›¼¬?·ª°~á¨?¬à}2¤ö?±â÷ÓØý?£+È6¹EI?ª¨&½="‰?î±]þìbG?¯ù¾ƒš?6qÄ"
??}"÷¬b‰¹?›99ƒz?‡s84c"Á?èC[Q®?¶p8²!¬?»84Ëtï&?­çÀß|Ôq?ÁVy-Y¶?±41NÆP?ïøkç?BëVàÂd?6=
ìð‹E?6ë_"¥?C5v …÷?8ëýþäëS?ïg ܪ¢?¤VK˜Þ{?"îÇäÔ­ ?¡-ØüíD?†È§ôÝ)j?ŠVMø-0?ïV+9ƒs+?' tõ`lå?S˜ðÄ$?t:ª:n˜f?ŠË¯GT&?vÇ¢`{?í|Ig°›ò?œíõƒà?§—‰ŠMC?'J§+®ñ? £àlØ>?'úÊWB*AGN3FGL J1007.9+0621@m00ÿì·@Fÿì@/šøÀ8õ¬Á"ŠfÀ;}X¶zzð?ï½ÅÀ6@Aé;îB¾@@<`ƒxp¿ÚIÿ6Ô¿å9=–ìô"¿åÈ,Ì礿¿ág"j´AGNbll?ïæ©zÀÄ	?eN
]Ô¬ø?^¼²•—k?^Õ÷<E?SðXFUãV?S]Ã^÷ͦ?ï8MñœÝ=?¡F}¬—è?ˆœÚ,6Ý?"»}{0&?‰O©l'¨Î?•ªªBq/;?îßÌÐJ†?;}8ø¶?'ŠÅýÔ?…HEÝèz"?'{·?ù"u?ƒÚ—Å"ÙE?ì¾Ï´Ú?¨"÷@‡½K?ª¹{±-2^? Š±Á¥ô"?±µK«€õÿ?£øO¯ÜR?ïô!Ó´?S±¢'EP?O¤!Ìõ6Ü?Ll^i—I??¯ª8®?;ðñFɸŒ?ï¸FŒ¬â?ƒs±"ƒTâ?rS€±œià?xBuW)?q‰9;î=??xû[¬'S•?ï}F6Ô?|²a£)Û?ŒBé"?uÔꍲò?~Î'ô÷?o
B«KŸÈ?îËí	5çK?"¹7Ēl?–úìª>«­?^áᅎ?ähW©Ë?ˆãÖ|ïèAGN3FGL J1008.9-2910@p"íà
q@5cÿƒÙ>À:.'Gl¦À;ÄÁE°
y¿×ÑkJ¯Y@ÓÆØA/@ à"ªÇ¿ìD]|i¿ãèPÔXÝ<¿Ñ»:X–o¿ìànà]xVAGNbcu?ïÌ~âøÍ?­íR&´ð?ŽókÔÌ?¥"{>µ~o?‹Ytv°œ§?¢ÈVRi{¼?ï5Ùñ‹&?–5êÑ"O"?‡Ÿ·–œm?'0¿i¥žª?Šê_'b-?ì¶s°V?ìý4·º?¥‡lùÜ?²ËŸ¸-¿? m·"	f;?©ïK~â?˜5Â'Ùî?ót½}?"Uh­·Š{?~Fpõ²?ysž…Ö?¡6‡ú«oi?'Xuä'ú	?ìò"Ãã]ø?ϙªo™"»?…á_7/Ò?¡½lKq‡F?µ¯­ï´OË?Ï%¯MF@?ï¶{¡®]m?{e	Ùðd=?p'"\)áÐ?bÌa¼NS?t0šºÉo–?vDöÞÿäV?íÉñ0ŒîC?šMXÂn?§w¤0´Cb?–™"E"´ÿ?—Ò'"ØèÏ?‡éáý?ï­°¿Gv?rçÁƨ?iŠËY´ï?]ŠÖ7x ?|³Bo‰?k¾¶ ñÀ¸AGN3FGL J1009.0-3137@p®…×E@3¥Ð]óÑÀ9¾~ÝU±À;jõ2F¤)¿ò\ªÈÀù…@BN¨Ú@ÈŸ~µé¿Ë×íÇïz¿èn[ø¿ã=;þ¿àáH2¯æÉAGNbcu?ï-³%ô?˜'dy¯Ìê?‡sy©¢ã?Œˆý¡Iü?F™šÚÝ?Ž½ŠÏ!Fê?ïV¨`åP°?¡'p¿'?,?væQXõ?Š‡1œŒ?ŠštŽ[ó¨?š"nÿ‰"ñ?ìzfv'?£_øFù?£¥'ùø‡™?'xÎØF¦Î?²]P™Š%?ž`ƒÜ©µ?ìbj¦çá?¨)îL4'?l™!õ¬=®?joQ'
Õ?¼
×2ÐÒ?¨…,¯sf?ïÓa+òÂ?w@¦¦Vó*?d<B
]œ?ph@ÿÏ+•?hbÓþP¼?i:j¸oC?ïÊPïdYú?4ç+"?eT Õ·?dÑÁö|k?pJ^6ƒØ?z>†z\?îÝ=¾§p?‰™ŽˆÑ–?ÈÙZ÷2×?Šñ'P–?"xk¡Ž°‡?,å1¹´?-£ì?†¹×ƒˆUç?IÐÝDÿ?AL	¿E
÷?>óçi?†yÏ?fôáAGN3FGL J1010.2-3120@p®Ñ`4P@4
Z?çvœÀ9˜
¨_/À;"30®ô¿Íš ;@ÔΎmìm?ù8}_|<g¿ï–`p?ØÝ|v·Ü¿±ëSBÃ#¿Ð9o•í›AGNbll?ïüå\bU?>;>Ñ"i?ê̌Ȟ?¿ê^î}?4mÔ²d?<Žz¼g¯|?ï³xt…ä?ˆÎ]ÃÏ?o?Ü=ü?'#)Ê܌"?v»#Éà¨?|/°AÙ?îI"ò‡?œ`¹ß?"zaBs?Ž¾Ìtðê?¡±×#Îø\?–ç¨â?ï…Ù©‡«ä?ˆgå{÷Ÿ?1¶÷¸^æ?3gˆ²˜Ú9?ûÝÚ±ÔÞ?ˆEGTIЦ?ïþ|pW?'+E·üp?
SϨ•ø?ñQèч? ë%í,ú?$J'lu?ïä´?b@'?f6\&'L?V•äÕÃ?R´gÝ&:?`@õ´'³l?`4/
à?ïÛ

†7?'¢{јʣ?‹Ý–æºHa?‰½ÀrÿÚt?'•ÓL©âù?Šµnóc÷?ïÚÅ(=¶Å?cšçØçA?*‰Èþ?!vH?ÒöÇ?qÌǚ?cF<&Û6ÌAGN3FGL J1010.8-0158@nl»À n @DÏPßìdBÀ:+î^íÌ!À;ÓN+>?ÀU¤)ó÷è@⧊Hò@	4¿zSÙ¿ãè(b}V¿æ!\?µ¼T¿ävÌsP¿è4í™1PAGNfsrq?ïú–vEù×?8Þ³'à˜?0‹Âý$]I?+H…FÒªŽ?:À‰R8®á?1}n5ܔ?ïv€ò¬M?PEpU0<?zRm!¡Ôf?v¿eSìd5?…6ŒÙ휦?‰Ü½"pv?ïjòV
®?|Cà×}I?yã¶a¾y?hÀg"ÞÑ·?ˆQL‹4V?ufiqUÔ-?ïE½,#}?‹¶·¹x?€îKÇY"?p²1×}Õ?–÷Q;ÏŠ?ˆöÔvþÿ?ïý}Ld+?**Ah_¾?"þ¹½©)?DAï´?&9֔Z»?!B:CK¬}?ï×ö—Ý'ÿ?iN·qÍ@?b<ê'}?VûϼdÎw?eÍVÿýæõ?dTzéʊ?ï¹®_No$?p5A?ºN÷?lu
éb²º?cs\9+
Á?tîIIúà?hèG1®×ü?ïÍ+}ºÉ?d-7Ö»ú÷?e|Í
jóÓ?Jü\þ¯.?mjmû
Ä?`ȶ{FY@AGN3FGL J1012.0-4235@q#,ÿ§ël@&kþ>^à`À9ž9Pƒ¦À;…§ÉÞ?ôŸ^<vRî@
9""Ï°W@9nà2…8¿íytí<Ú?Üÿ<ÊûU:¿á~ˆ²S[¿î
Š°Ù¸TPSRpsr?´ÑhFá?´?îé"h8?ëóÛ §³?»†³Ÿ,3?§wv{~É?©OJ½~Ö>?ÔÊZOC?³Q¡¸a?ë—Ðc&¸?Ä$69¼©?¿®ä§èo?À£L&Zmñ?Õ
D²È¥Ý?³ß|Õ»T?àøUú?µï:~Í?ÂuFh_?¥¶=ïBÑ2?»w>»Q¥9?°¤´"Úˆ›?ë5–!6}ã?¶¡.I7®!?¥¸ yds\?¢ÛŽž£Jœ?½úv±Àµ?¸\'‡f7Ù?ë&Ü'*2Ñ?½nªôµ…?£lHžAƒŠ?£Ã?决?²wÝtIYä?»ÚïöÙ¡Ù?ébÒÌÚÓ?ű¿S6ì?¾…ùÌÁ?¾L›dc?á™i¸ÖJÐ?²`Ñ]ø{?Öábq gz?°‡Wu"e?·¯(s9ÿ?ÇàÛ«?Ó¼®'_w?µ°eËÒJ?äÔo¿F©?·P-½"—?¤Ó'ÖN±?™M¤öƒ¼MIXED3FGL J1012.2+0631@mE:Kâ@G?µ!µÀ9¥"÷si"À;"ÿ·¿ÔGpõê @ +Dý5@›{Q^—¿åρZ]™Ž¿ãþ À'¿â©W'Á–Á¿Ô@ßu"AGNbll?ïóša"?OÌàO¬×·?<êÊ#Ó+z?3G•N\¬?Q'#|§ˆ?K
å ˜üª?ï¬ãª×&?"vÊWÁ£Ê?qfhœ2è?qÅ"Mû"?x'©8ßIÆ?_Kjc­n?ïR¬¶4Ž?~Ï7s$^?ŠÝl–Ñõ?l=™lcÝ ?‹¹æ)åã'?u¼0i­Ä?ï:Pù—±?ˆ
LÕ×ɑ?W"ÒîlŠ8?U—¼K˜,?—<£Ÿ$Ø?‡Á\Ä5«\?ïü»-¤9?2e‡»u?(Md¤±Ñ?¢,n'º×?2ûr:¦¸E?+ Ȍ›î?ïâàÃy½?d©ðúâˆn?[Ššû$î1?TiK=Ù?`+Ò«û®?\2šr}?﬎¸Xæ:?er¡$º£?q|'UY÷Œ?Vt"ï"6©?x<!‰á—i?\S†¶ý%…?ïØñ¾sÜ?^½ñò†ÿ¾??²$n;?2&œ!E?q‹þ8 ®?]'Šc"!§AGN3FGL J1012.6+2439@iøn «†@K+|à%o%À8=†Ñ™»À;S=Êeê@?÷¨¤&æI@WƒsèZ@ïJݤ¿Þ;:žaw¿ä.ŸJç¿åؼUl¿ìК›»÷AGNfsrq?ï"a§muW?…8æåøxê?ˆ±íÜ
Ó?"Ì):–;Ý?S­BbäóR?Jº†JÈ«?ï´·y¥?ˆ6˜Žg?rŠð1F"?'ùŸÒw¶?s‡.=Æ+?w–!°Ïú'?éjT¸ûø?­ÕT˜¤[?Ä{2Ñ8—K?ª©ÌHK?§mé'ügR?™«Ü\ú¼P?ïÕ»"ÖCÄ?}BœD]>Ø?R§G;ï?a;ú-ãP
?pxœ°b¦n?{¥Ec}N?ïPËtˆ?"Ït.ìu¶?†ôÃö_Na?"möùÜ?Kp"•£ì?ARC»^ïÞ?ïåêì-Ì?fî»LƒNœ?Y6.ÛÍ« ?Wú–Wsã?\¹û£Ì»Á?[ÏU‡€ÆD?ë†éˆ?©o«ÛíO?»o©ÊØð‹?¤ø" ç€? À=ÜÕ9 ?"z	Û¹?ï÷&¢¬ì?UHÀŽ%D??ÛØ5AýB?EbKHÉýé?Cw‰^ß]?PŠÐÞì=bAGN3FGL J1012.7+4229@fԀu@K3N?þó'À:r±ÎCÅÀ;¨¬¥åØ7¿âb¡Úà%@]lWA/u?ú‰ ¨+®¿çþ¶lÛ¿ãñðPh+¿ÂOw݇/¿Ó´í¡ÈVAGNbll?ïüz Òj?;çVPÔ¨?7A'"r?gi*¹'¬?:fcYxÌ<?8f
êy?ïºÊj-+˜?‡­žtKŒ?nÉLùÌ?'ÐõFu?s6>]
Uš?v¦9pÕ!O?ïul¨
¿u?}Ú3`'#?vÙ)#}D7?d•¢"l?‡8Adú*©?y¯[†'9±?ï®å|'BÌ?yýj¶60?&r뺜?-ðX`	]™?ƒìØÅyRo?yÆþ¦ÁyÍ?ïþOaoº+?2³yÕ@¹À?
xë†_ôÁ?ν'šåÚ?#«±'¸o¸?2^رóçz?ïèè¾3ƛ?f5ÀHˆnŸ?Sêð˜ë´?Qý‰ÜvÞ»?ZC"W}Þ?`äØ7á,#?ïµf_–¤®?lê"o"­?n¡YîfÛ?`Ïä`ê‰ø?uüE(²µw?dÂʯ'	h?ïïø¦Íè3?R*O¼XÚ?ë¢j R
?5/˜¦?^ø5Ó@ð?Q½Ì.êcAGN3FGL J1013.5+3440@g̸`™Ë@KÃC hÀ´À9Á/¡®;À;ÐsۍZ¿çنO@  ïX=@þ¸ Bj´¿áLã1£¿êt@;%è>¿à
ù¼«'È¿ïûàˆìMFAGNfsrq?ïóñëÙò?Uó<ˆ¾u?B‡æ5¢ýÝ?Q
æøÐF?M°jÖ?H,¸¼VAÍ?ïW§¶Ç??õy`¶pŒ?…v=­x?€«›®m?"ŸöOß³?"çú•Î`?ï[u`n?†÷î.^q¬?ÛÜ@O~Ø?}³;­à`n?&£5'K}?~uZûo;¾?îÔ¼
ž	|?•Ç•õ-Ä?ƒN}ïø~Š?"¿ö?›Á?Ux8?ú&<ο ?ïÙ@}k,?¦œ2"­x ?qˆœ}ðâÔ?¦ þÝÍ?=rL ~ê?8ºZÂh¬"?ïÌvh‰y?s[Y›ì?i¤¬Uª?d0‹RIôú?jRÝ\Žä›?iÚ÷@u?ïhöÛá_"?w›;šáÉX?…®®Æß?q~¯Ð>$?€É\¿€?iúȤÇ9®?ïÏÄÐ÷KH?lî,5Ï?W#HœãcZ?QÁ¤v
™?rTÅl?Ë?h¤oÖ¨÷AGN3FGL J1014.2+4115@f\ÍÓØ@Kwÿ´€¦À:a)ë‹ÔµÀ<‡ð#éê¿ÜÅèéMY@æ?Ns@c¥ÀnoŸ¿¼UÙü5E1¿åìÖÔà!¿âì/a¨¢²¿éKÍ&¯AGNbcu?ïЯU(ã?U‹€±Ö#?u
)T8œ?€Â8^=:…?G;÷%Å)Û?H¦ˆ'" E?ïeb¨ÊA¶?'j(ƒíi?'f±†"Œ?"þÙsÖá?"@¤J£˜p?†ÌŽ"<÷Ê?î
íLj?šÌ6c(?¢@qh°À?•h¤Åvá?š!yy
B?…!rïËOU?î¦ÔQjD±?•Þí7…»1?‹aÎ|$hÀ?€ŽùC?tŽ'íg~?'êA8Ջ?ïóY¥U?[åôqǏ–?T·Fםx?Z'_þ‰Ÿ?2U¼}>FŠ?+ïv²î?ïÏÚ¥A\[?sûã]i8?fAf;À@?cÞ-$TãÒ?iäTÏ=Œ?kiË(e'n?ïÖnâi?Š‹OüXî?')ÊB£-?†¥äÓ>Å?…6Њk?u%²c4mÉ?ïŖJÚ*?ncÔϑT?dòœå?S©¯Wñ)‹?s(ù:qY?j^iàH÷AGN3FGL J1015.0+4925@d±?Ýe¡@J[‰€Fâ=À7%cèä÷À:5›Jt?ì"$áûvó@э7`"j?ýU®€0'î¿ÚªðåÁ÷m¿ÚÔm®6è'¿ÜŽHõ¿ÙãÔåŽÔ]AGNbll?ïÉÌ˱U?±à
Ö?La-|šò>?MÀ­Z^9?wtmsI›?€ªcýf®Ç?ïnŠC²©­?™/ß¿—?ßv^7:?…Põ+‰È?'}ù£s?ŽXQBbä?ꞎŠê ½?°Ôÿ:\?¢ÌËÅÉ;?˜žÄnO?ÀҒ㶷ü?­wOȲd?è5ë‡"·?´KE"Q
á?˜#‹¾A?'‡˜?pf?Ì&ÍrÑ[?´vxŒo?ïíJûÉ1?b6ó"×T
?AÌîÉq9?B½P7
è@?\ƒÑ•ß?_n¸#ƒKÿ?ïą²uÍP?ƒ…Pþr{»?lܵõ†.¢?wðZ\I,q?n—h±,?w¦0ÌÈD?ìÀ…À"?¨eGÅuòI?œÔý
€rá?•tN`ª›?²Æ'¹ëž?£­5o ë?ìnDHPÉ?ý3ï\?'@DÎ#?~äÊ÷âވ?¸­"¡?œõžåŸ1AGN3FGL J1015.2-4512@qC$ÜY2@"ÊÊërªÀ9î"
>À;•¹Ù«¡Àð'äÄeJ@‰ý²rÙf@é4Â='¿áSó:¿à
sÒEí'<|T‡?×ރi½šAGNbcu?î\Q'ƒ?°¸Vÿ-V¬? ýwÆ}V?§æ­êü'?"CáÐ@Ôï?¥##­š‡Ÿ?îŒð«úa?µ]•_â¹?u2àˆ¦?€#Î	€#?¤Š™<?´äê|•?ìÙéÓãÜ? h1Þó‹–?£Ÿ‹_¿å?'9Uê ÐÎ?®áÐ9ÐV?˜÷)­þtr?ïâéÑW?nÃbe[í>ÛzL¢Ñz>õã®a/þ%?mqÜá?nºپûc?ï¨'jÁ٘?'mU1Ït·?tÀ¯·+
"?ˆÏ'Ç>ø¡?w+šè˜-?~åƓVÅC?ï §ðô€?–d ¥ŒÎ?_
½Ÿ…?fšJŽ'…õ?ƒô¬:Š-T?"¶¬°êÇs?î·DZ«zË?'^Ã`»¢E?'-	‡ï÷??"Á‰«B—?–êk&KW?‰l=)¦ùq?ïûËmQ<3?AÝÖHÖØ>qZtºÇ>šðÜÉB?@ÐT@qþ¬?A@unOAGN3FGL J1016.0+0513@mb€'،@GƒüõŠÀ8K¯é(À;)€,?çAÎüýÂ
@@–Ì_¿ƒ@õß_÷av¿á°à.m?¿å»WeÜA¤¿Ü÷¹èø¿ãw×èè>÷AGNfsrq?ïþ[M½?"_m¦'O?Ìo
®Zy?>{?Çf?#÷F#?'òd_hý?ïÀR(Ä?~ÈÓ®"Y?l|:"ò·?nžnìÏþ?qÓù¿"œÖ?uÜÿ
Ÿ ?ïxs¢A¼l?}r½ôÚ?vh_"ñåÀ?h!-ÉP9S?†®çá/˜:?xîqÓNš?ïÂüYW_7?w¢®j/úg?4,ÏÇTz?C	.âG†?}?sŠ,é?wØrg¼€?ïþð™ì¶Þ?f¬•^J¨?®Öø\?eHdε?•_Šœë?EN1u‡×?ïæHqçW?d—Ý°‹Ñ?VúyZYÀ?TÐšp?\úöø"?[±ÀœZÆ¢?ï²*ŸÔy?p¿ë›iß?mïíUì ?`_<à2ë?wò¹œÌ…{?k/£š›£?ïòÅëdÆ?R·m•Þ?(v$8Ø~? ªgՊ?WqzÕ'öÿ?R/èzþ#AGN3FGL J1016.0-0635@o"ddIV@CÂb¿è¸¼À:A/)¹6îÀ;ÐìwŒÿ?é˜O·Î8@6§µ\™@Z]ÿ—¸?ŒóžGÔ*¿æ*[—ö¿íK£'è¿ïÿ°FP¾¬AGNbcu?ïÎ5#'8?ðpQ‰ýö?rz»dœñ?|'Œ /µx?YªÊÕäì?a½Ñ®Ê2ˆ?åÒi£v?ÈdÀ´e¢Ç?ÎÖ3¯@0-?Å@r÷)©?³ÀK…Ë—ª?³"lØ9î?ìXKü,áµ?£+ûc;£??³ËþÞ9S*?Ÿµd̆ž?¢ãB…
ÁO?'Îët¨ƒ?ُÐoÍ ?¼B8LUL?à¯ý旛Š?Àï%߅?´CŊÍÉ®?§"œï4aÏ?ïË?ðõÓ?'OÀÓ1zR?q׶ëN#?‡*×4¨Õ×?a¡cîŒ?"WrAþ‹?ì¿$æòÆd?»h%Z?²œKEcÕ?¸²
šžãl?ª4á",? ãŽ4œ?íußnv;'? É}ºzkª?­ã"f3M¦?›ã0üðù?•|éabX€?‹Pïéü²?é&u"Îûó?¨ÌÃáj?Ç@šÚŒS
?§kŸÿAòœ? –;H
¡?"½ÙÈfiIMIXED3FGL J1016.1+5555@c'7¼]ê@I' ("tÀ9ÿÓ3[AÀ<Š7üÇ?'Ž»Á¢ý@×`Ô+:ì@3Úÿ•võ¿ä>"èÚÊf¿ç>y|1˜˜¿ãW{¥ÎíJ¿ïÿÍ&}±öAGNbcu?ïôŒ¿õ¦?T· Ï°"?9l\…v%é??gv_/ç?P‹hmðzÿ?Q´Ïû·c2?î›rt'¢T?žéÒÇ+°Ú?™wVüûŽ?'±E?"?"Ziðîò?'¤¼ž'ó?ï(ü•à?†j®°¾4•?‰µÝ`>?!r"?‰ë?ˆâ'""7Š?wìuGùhŠ?î^¨¿§J\?—ÞH?ûðæWnn?"S¤­Þ¼?–.÷)æ°?'»ÎÙ´•?ïüGöµÿ??À~lj´Î?#ŽNeôÙ?*LbüڄI?4WͲ?6±‡,a"Ä?j)¶Õ?€H–I«<?|ælN¾o3?u‹P•îŽ?uÆÞ³Ã~'?s¼9tõY6?ïgÞ%±Ž?y&îHª?‡"ÿ&üê?vc4óɱ$?|èï·6è?e‹'#¥¡?ï¹oÛsó?r—f³C0þ?vnÅɍÿ
?c@Óñ`€J?j!i"–Â?j'üýX94AGN3FGL J1016.3-5858@qÁUÿæՍ¿þMV¾|'À7s­uïpÀ9¢ì,
¥?û&…}'âž@¼œ®L9@GÔJDœ½¿á¡—Ú§¬¿àÒ¡'Ïe¿æB°ÊkQ:¿ìU}ÃOJ–PSRPSR?Jž6W?G©Mà±Ò?àÿ‡7þZJ?ÌìØA0]&?Ýó©Á– ?ÌïizS?jî.<mŠm?{+'§?á漞<§·?Ã%eó­iä?Ûüªf¥m?Ã?/ïöŒS? n,½Õ?''É\OÃ)?â¾}ñ_H?¶ÏÒÔgÔ?Ø6W'¯?µú´ÂŽH?…²E²È²?‰M«‹\á?Òþ]ST0?¹ÊUÊÈ÷¼?åü£ÃØÌ#?¼­Ññ
*?9ŒÑ܅ݭ?:à×OŽª?ÖlšÕPKi?Î(ù°?äƀû=" ?Î¡õ™ÛÅ?u[SÚ
û0?6ý©IÌ
?ã/†'Ìͤ?¹›F
.	Ü?ÙK†`×±,?º}K«á+?¯®\2'\?¿÷9'á?ቀ²B?µT^3v€ä?Ø÷3Õ5ž?´V ¦¢Bj?Ž"MsRƒ?`ãÚ*du?Ô𶥲ÆU?´òµò±1?å
Ww=×°?·â­2v˜MIXED3FGL J1018.1+1904@k1  ôØ@Jýb¿è¸¼À9³e·ýäÀ;§'ûç2¿ìŽøjNAE@ؾoçÄu?ÿ¼Á¿}ƒä¿ç2lw*6"¿×ׂÍ2¿ãøãÊ¿²ïæéiÍAGNbll?ïüÝfom?1˜…ó~U?%ôŠ¶9ÓÚ? `g¸7ÌÅ?4ÆÍb½)Ê?*ÉCù¹*o?ï¶rôù¹?ˆ©Ê¸LAŠ?p¿¹ ã?ƒìM‹%´?tÌÉ®÷…?uè©Kÿå?…²m6?u¯ ¡­Ä?yD#Ç6?n'%£Ôä$?"|…«àÍ?kc'03}?ïËeÛfÒ?rºßÅ»÷?%(p·x&Ø?(ŒG'oV?y£Ï=¡¶?rœÖ/ºe?ïý'
Íâ»?'šåàZáó?åIl™Ôý?˪q垨?&ì€ëqѕ?!n?1 Ä°?ïçÈ+¦?g:¡4®?SùIœE	c?R+4).úÎ?\v~f+®?b	w;åx.?ï¾%º¤¬?h}[¦ëûà?obZÕnõí?dQ£ÉæÃå?q;õ0d'ú?T짃Ë$Ï?ï÷ÜqŸCk?GÚ³
´×>ýÆ×!!ÙÉ>÷ƏF*N?O :ˆìõ?GšŒHAGN3FGL J1018.3+3542@gŽï€Uûµ@L:. &{•À:,G"GÛÀ;ç¥b$¸F?â³Ôœ±d@äDó¤ýÑ@d'Ÿ¥!b¿åŠº3 žú¿çë}®ùÊ~¿åË©tX¿ïþq|ýAGNfsrq?ïä˜]¯]¦?¤‡žÂó?#mmÔ2^"?%3¦õ–ƒ?j0Ë©©©?¤ˆ~m¬?ï/Lœë…?"ôÊub5]?ŠªÄrîâ?‰Hý8¿(
?‰'ƒ÷Ë?Œ—•³[¿?ïµ2/Ù?ŠlÅ
+ZÎ?'=F‰0¨°?"&éÂ?‰X&T{?|ý4n%³R?î]š¬5 ?›ÀÛ­fŽ?Ÿc'Uþ?'Ê'l3&?"ü=‹xZ	?è#c‰°?ï¶npÃXý?¶‰ —Ó…s?_
5ó§Ì?žõ`nô-?}z )+£?²c«r `§?ï·jä¿ ¬?xšnåÀ?r"%Z±=,?jÖ+è?q·h#bU??pœyVXÖI?ï?µÙQ{¯?‡'""F?Œg:"þ?'%OYê5?ƒ'ì<×\U?~"ÕU§
`?ï"+®À®?xú	ÈâüŸ?"ÒâaÈÁ?nuë;è+€?l¸ˆˆ^é?oê	kµAGN3FGL J1018.4-3119@pÆp_®¼A@5!@ÂgïÀ9€÷¹à`þÀ;ëg†ù?ðzÁDXt‹@¤æÛkÌ@D…ßÓdÁ¿Ú̆žó©8¿èsá".c¿ëT³Ý¬\Ú¿ïôf¶1C´AGNfsrq?ïz8ÄC´?'±Ø&¼?ŠüMwæ?'F
:+ð?i×­ìƒìŸ?h¿›ÿ¥—?åõAŠ†M¯?Ác
–k'É?̊竆'<?·ØÃTÚÌ
?·@$WT#?º7L®•\?ì¢Ê•îqì?¥èŒˆôaº?±r¨cää?Ÿó@î¡w£?¢îÚ|?"AJ6Õ¶?ݘ$òÜ3¦?°ãQ&ÊU?Ú±µ'"3ö?µ?ü­˜²œ?¾Ø•î>a?©…ï~¶¶?ï½£0?™1›¬¹õ?{æcr¨U?}¢ÿ±"?U <úð?Q60é¹i?ë㑌|G?°å[¡×Ï·?·>~^ãb?¦9)؛«û?¢Äj72D–?¥·ÿ'?	?î_b"Èõ'?—+cDõi?¡‰ôžV?'Ý\W'å«?'m–Åú'?'G›ÓŽ;?èåÞqâ?¡¸†UÛXö?ƽ{
¸?Í?ž1­~°?¦¬,Áš·?" ì$['AGN3FGL J1018.5+0530@m–/IŒ;@GÙUÿæՍÀ9V‰µöÇrÀ;S 'àð?ñêâצ°@l"6Ûß@ΓÏ,?îMKMV9¿ã ó粛¿èk¡—ÐýÅ¿ä}å-AGNfsrq?ëÇóy‰Ù³?»Ë"Ëå>?¿Äz\¬B?»Fð·ü?…üýØb¡?ƒÃ
´k?î
j';?·¬4 ¼;?£X÷Ѩì­?± ®š^oà?˜llÑÍJ?§òjšll)?ë@Sç!¦ˆ?«nš˜kH?¹4–ìöJæ?¥j7§ó4Ò?©'"¸D"³?—uEl껪?àýÖ¨ÿÏ??¾'™W ñ?ÒD—à˜ô?Áõe=¾?ÇušÐ•?¸ÈØkˆ"?în6òZzö?±ôÝ¢äÅ?¥"Ylåö?¨7[åBµ=?|Á¾Æ¸­N?«tÇëüâ?ïùF¬?­=˄Ѡ?''¯Ý­å?¨_쌡2?…ELŽ™£d?"­ñÅsŸÜ?íà4fË!?›ÿ³ë?§ké;¦ó?–TÒºBI?•&'qkã?†Ì¯¼@?黓z#e=?­éŸ¥Ô
Ô?ÀØ¢¹'ÿM?ªxEÿòÄ?°r¿(Œv?¢£aåRAGN3FGL J1018.8+5913@bî´ßݵ@HJa€M˜9À:ilØ{À<&¿è+οñ~:Ãu`@ȈD‡™@¹,?Î÷õ¿å›Z—ŽI¿âYl"=·¿Þ^…Ø'Ê¿Øó†FÍç!AGNbll?ï÷®<5\Ñ?Q'JyMWL?<=Y]rôó?AÄ®Žøë?C(b¯€–R?GåeLû+?ï´ê²Š#?€§Ç¨^«?o
ð…;!?p(sÌYû?vw«¸¡?yž( 6Y—?ïCÓg×»Ï?"°sÿã¤?†=÷XýÍ?@¨†o?ˆñèâM?vNۂ4´¦?ïâÁ2å°s?gô¸ ßÉ?"F~(ùÃ?$RsFÂ'?lØõÅTŒ?f¤Ò–"t?ïýyÓß\?3Sm~,ð!?Š4Êa²í?üa£Š¼?+«¤ÞW?/Ėëdøˆ?ïåÍÄeíg?hhO«T#8?Wœ'gdFà?Tâ<uO+?\Çå¿{?b‡AË;(?ï¨Ê@¢ÔÎ?s¾+"ÞF[?u°‡ÊÅ?n°þ6
š~?v/̼=?b"A"x'›?ïûä)µ°ü?@Kn.z=¶?Ö¨—Ü>÷QÏ®ó'?>»v$ߏ"??ü
"¢e0AGN3FGL J1018.9-5856@qŞ 3玿û
¬RÐÝÀ6ϽBNÀ9'¤g¡Ð@lá//m@
ô܄¥Á›@òƒë‡x¿Ù£ôüÁ²¿å¯íÎ¥!¿ç¶%÷
ø¿íTš\78OTHERHMB?BtýWáË?EŽ_¿Ž¿?ëíMŜ,?À‹y™&µª?À8¹k,Z?À€êûOÛÏ?úØo,ˆ?)eåלžÜ?ísœž ƒ?­w)¥ß±?·xß=Qj?­wÙ¡äš3?q—ê9g?–òÖÎb¶õ?èéÎa'.U?µ yYH Í?ȵXF½ÿ?³â-
'¦?2ò0T ²
?4iŠ/½"l?ëÚqŒ¡[?°==ÏΝ?ÀŒÂ•*7ü?°~O³"?!Kî¨þS?&ÑDú¬'?ìX>¯àzK?Á/œ°z[¼?½5ˆYø'C?Á-̇éª? 0ÊW%ì?%gåávÃE?ì$ÜN±$6?®BrZ)[?¾Õ)…½ø&?®
¶{@'?¡£_Æ`6?™ô¦ûÃ5?èí,ÿ˜"?²7¼—»?Çât@'$?°íù?1ÝJ;t?2ŒŠ-¾?ì 3%¾¢à?¨EŽ^	ó	?¾ì‰Á	u?¨JêÀ¿PSR3FGL J1020.0-5749@q½ž 3玿åeSßÙ¢|À7¼ií£ùÀ9Ñޜ)¦?ñØ$ ñ')@Ý‰ˆk@¦nmXž¿—?¨®×»¶¿ç¶®t¿g¿ä1yðºp\¿éc`!¢½PSRPSR?zhSŽbýÓ?vIÀ‡Qêð? wÍÁ^°?§F™¹QÂ?îò|"{"?¨›¿0ÿg¯?¡ÜqY¯Tß?±‡<=*Õ?À"¯õ¦ŠÄ?µ'àÑs8?ê½Lìí©'?¾ݗ=Ê?´RÙqV÷Œ?£I5^HÅ?¿íB83Î?¨	¦¨èðY?éwüŠ÷â?®Ê¥‡î
?·}'ŒÆN?°ç×Y›>?­L52Ô??šš"h{7°?ë;ŠŒ­ÅB?´áu¦¸J'?…V…1}‡‡?ŽµÔ6Wõ?¡È>Ñ)±]?¨yøÔèz'?îŽ!ýðu?«ñž¹8-?°œ©Gq
?¸³.¥!Z?ÆÓWH™Õ\?·¥ÑÍqö-?è7§˜y¢È?ēq'ЍÞ?½Š3íd¿??§Û6onF?À§íÿ;MÎ?§VÃDº?è$¾?°e}£½á'?¾õzbi#'?¸ñåÛZ'î?¶¢V}­Š?˜OññK?éMñugz?»L¢¾—'OTHER3FGL J1020.0+6323@bK^?»×²@G"_£Ô†À:+)­xs¯À<ìÀˆì?ëó0Ùç'v@
c~Ì
à@Kø`îW?î×·¿D=¿ä^häq¿êY4ð¿ä|#È9ȬAGNbll?í³£‹_ð?¸TÚl°ró?®ªQ…/Š?·Ä?'ª‹?ˆn×ì>à?†NÝhʎ?ëŒ!õ¨?Â瘦»§G?¸*×&üŠ?¼äfOüC?¦è@^©~u?²øTjœsA?ëÁšÏÖÿ?¦¾Qǹ`¶?´&­
\?¢
Ʊè‹h?«àRcÆb?""š.@º?àhn(}?Æå•y,?ÚQC°y?Ç,¾ö†•Â?¶b¤ð":?³ì7€‡À?ï-®:ª9¿?µGŸ5Ù¹l?•]ü¿Á'ÿ?µ;"©æZø?s°ï£È¸?rCX¡*'^?îuJ9+'?²D|pcÌJ?Ÿ
^3þ9u?¬Ü,.dÊã?'QøsZ;? %ú•¦Ó?î¯Íì;?™«>u?¢V"(µø?"]¿$¢ß"?˜Üýù=äª?ˆ"p:ñ/½?ëÅ/ӓv¦?¬boyÊE?¼‹Ùx½è?¨,"ç
ˆ?•*Ÿª™Šð?•ÊÉqäÏAGN3FGL J1021.8+8023@`@Iÿ'ò¶@AKg€AÙ¿À9é-¡"ú×À;ù/À·ë"?êÀû1Ühn@_ih¤Y;@!@—tѿ吒fõW…¿ç—nµÚ¿ß9,"ç
ï¿ïÿ±žs.AGNbcu?éð0\ǵ?Ê#[yÎM+?²…¹u;8?´o2çk±?¹b"&Q?ÇðŸS±œ´?ÀÝ~©[â?ÂñÝCx¶Ü?è‡7¾w
l?Êca›Í'?»Š‡ôÜÙ?ºÍcØcü ?ç?Y#ݪÁ?³ïIŒV‰%?Å¡¡ñNY?°e¾ÜmUx?ºÃ0
J?¢Ôþ/×oN?ڄ,ã–px?Àk«³¢"?ßÁ7"%?ÂR
`]/?¶êp
{‹?©úSÑ_ð?ë(»R8?Ð0ò#§À?£–>Å]xÉ?­¸ë¢§?¼ôªÈ|AU?ϑQžbN?ÒñŠê²Äl?̪[7Fœ?ãÉûê¥-?Ìÿ;J?µéôÿŽÚ?¯Ê璝g_?ë½R˜dw?¦ùÒWdæ–?µæþ'¸'¿?¡;¢l¡ÊÞ?¨`}Ôx/?"V±-w?æ;×a²€?³ó:}Êô?ÑÁΕézœ?³‹ÞZ1?œh6€Ú)?‹ÈÊø˜MIXED3FGL J1022.3-4234@q<‡¿çáü@(š"ÿ%ÀÀ:Au}Zž²À;¦ÝÉtR¸¿æ¼ ÜGØË@Q®Ÿð¡@° M¼¿é‡wÏU¤]¿ãÓ?
_ˆ¿ãn,\€¿í¬"Ç
Ò'AGNbcu?Á™½×?¤Í‹$"?›£]þèò«?šÄÿ$ÃÚ?'¦éÔ¾Št?•ø3ðÌ?íùÓøÝnR?°·´EÜ?Ž6)RvÔÏ?"Mao¢?¨Õ6C3©?­'W«¸€?êzÁê=…?«M*}ˆ¾?º¢å¡¸'?£î–f
?±‡¢ã~Ç?š_û"3Îä?íÝÃ6ô~?šæ"Å&Y>?"{‡q	=Ó?~͎ð—O?­꾂å¬?˜Ú
_á}c?ïj¹×&Ã?'ÿ'šäØ?Š	¼ð a?†ÏõŸt'?vò¸£?"u¨8Æ؅?ïx3lWÛÎ?'€,"ºe?r L̈ñ?rŠ)Ï[AJ?ˆ¢ÜÍñœ?Œb~†«?í|2A,u?™Ða¸Éãù?ª"´â¤?"ðRÐìÈê?œGrk"ˆ?…é)õ}ã3?ï¹pN?v†L·e?ec
¤*¶?Xn~	ÏÆ?ŠâN5ºns?t烅þ«›AGN3FGL J1022.8-0113@n¨Äê@F0³ß•ý-À9#a.AÀ;p×%+3?èp/¡òóA@-hì'°ô?ýþjaÐp¿æ—ÿW?ˆ]Úü^ݿ׈ô'Q¿äö­Þl~ÑAGNbll?ïÀ"4W {?"?žÔj?lqš€V	?ptµ­ú?q…‹¸?{ÑDm"±?íg¿5¤@€?®eõìðs?©b%¹ø¦?¤ª2b
´? !æð›N?¢ØÖ6×"S?îzwàŒGL?'ñ…qwE?'åaã¿?ƒ»ÒS÷Z^?žË¢MíŒ?Œ‡ï'â"ß?éN‹¶¬úÊ?°¯%™
?¾pÄÁÌ¥?ªô+Ó¼?·ž…Ö]?¥Â'‡è¨\?ïé»w‡Bv?e‹\•±Ep?UHˆ÷·9n?Uc…µãò?W@ˆF»T?ZØf÷A}Á?ï(PøQF*?"jË	…
;?R$F"§‰?ŒêªÙ2
ê?…GyUR€?†|¬×l–Š?ïX(³R}P?ƒ§¾.¹?ƒ}•8€3ö?|?ë®áh´?†x=ú¥ç?x´|[Pú?ìב—ª?—iÍGGÇ}?²}}@ØÍ?"Å
û;+A?›çBè߇?…i¨¢AGN3FGL J1023.1+3952@f—|€"Þ@LlØà†8À9ßZ"‹ECÀ;䇀'a—?âk¬D}C´@~P¿54•@ÎÇà(õ¿å£€¢Ÿ5¿ëËåŠø†¿ïþ¥l-:?ïȧèMAGNfsrq?ïünҊjÁ?E±Á€H?¬ü¼­'S?58&G?6Þ*Ï]'Ü?DcR¯(7ß?ïÀe"ØÜ?ˆ
Õ¦M!À?pAÝËmÁ??ƒñÎJæ'$?o¿žÙî?qêÿ †3;?ïÓJj\j?†ã>à,Ô^?'€Žb³CY?u[Àà,û?"%O"rw?ƒJ'~¯Ü?ïí¡ƒë)?nÂ^–"­?1•Ý! ?UϽ‡}iæ?`´º®{vÃ?l¥—\2N?ïþsõ‰ô$?1ª‰Ì;?
êÍe'?
b9ÛC?"½ñ$v?/'ÊJ†cY?ïèë˜XÀ¥?fbrŽ	e?Vi+®½Ï?Z¥mj˜ ‡?W¿£ýtW9?XÆ&`?ïÿmù?}ÈT$<óÃ?uÔè
ë²?j·Â@Û&'?…ÊQ¶?zÇÓò8Ÿ·?ïþ·ˆºF?O±ç²¼+">ú5ò
úÙ:?  #`[â?+
ËnJ¯Õ?OY,ø¡³åAGN3FGL J1023.1-5745@qÂÉ?¯Bx¿Ù2ÿÔ™À6¢0'åøÀ9…{2¦Ez@Ïnc¨@܄¥Á›?ýp؍JUå?ìõÒL–S¿â#N+\$C¿çæ+¿1¿Ò¿ì:Õ_â¥PSRPSR?6ÕêR_S?4(¹;B‹?è -ëSSB?ÉkÛ	?^?ÍsÝ\çâ}?Ɇrå¯?ƒL—[a?5JËꕨö?çü1Mø'ç?ÀM$Bvêe?Ð/6EÚ?ÀN¸ü«?uW†¡‡¶+?sZ
w ñ?獢X7­?¹qÞ*}?Џ]4R[Ü?¸òœ¶¡À™?U
Ò­´?W¢ûÐjñ?å·1þ‹ó?¿a/¨o?Ô|"7V?¿P"c­W?!ᚄú¯|?#™tÖ1Z<?éùŽÉ~[?ÇÝóˆâ?ÈLsÝ-©?ÇÔô…ð½?5a¢ñnG˜?a'ä@Té?é3؀pcü?¶'/}mªX?Ë%í-"-?¶ƒ¥š?tʏØÝ0?{|ÍŠ{Í?çª*À'ß?´ü†ÿD5'?ÐX·á¿^?´í\i[²?Wýjw`À?WÕlwÝ:8?åÝêBÔj?µ¡u•ø2(?Ô-&~Ä×
?µ¢'uŽ~PSR3FGL J1023.7+3000@hÞeÀ¹™@LËèÀHZÀ:‰'³ò
tÀ;Ü&¯—1à¿ÉæM:<ß@
cäz=ˆÍ?ûîþ?áll¿è㎘';4¿å‰}AR¿ÀYå4ÞÀ&¿Ò§¶|d'AGNbll?ïðµÑ¢c\?U~&Tˆ,‡?%ñ«} ]A?"+6ék³É?[Ö'tz.§?Tƒ
Ã»ÿ?︷tÀ?€VTCMÛt?nµçûH؃?phî#/?>?tI‰°ž;?x¡gôV7?ï
yÅW§?¾Ÿª®(˜?'aa_R?ni'Š¿M<?"®)‰+?|.þñG6?ïØ!áôt?€×Rÿ'´×?FiPaÓjÝ?T‰Ô¥"?‹#bT?€=@Ú¾
"?ïù÷H).?>.Dzˆt? µSÖÊÃÂ? Ý×à•?CõŠ6m.?;ÂÓN‰Ø?ïççüCf?b¯Àº´"?W!Ä'ÞÅ?T÷kC1ch?YCQåj?V¤žg'ä?ï‹`°¼B]?oÙ=°¦†?voŒC\ƒ‰?bYç1÷d?ð
µ|Ù?e™—z·T‹?ï鲪Ñi.?YiíºÇ&q?=ë®Â–"?6CV¨6ÅN?bß8Ž¬¡?V¾:I
KSAGN3FGL J1023.9-4335@qIo@_k @':¢?ZˆãÀ8Ȕ¤gRõÀ;ìþ›{ò?Åëô
3î@¶b®ËÚß?üŸ[à{€T?Ülä¸Y¿ß]"–Ž]¿ÝZYOº¿µZeÞùlŠAGNbll?ïšT4_®?‡†ãÏ쾏?qáÉڏ8.?oô'¿j™;?€z
üÜ£É?'ë˜#&½…?îfÖüÚ\?°ZZ)m?ƒ|>¡DÇ?ˆ™f¨\~Q?¤³€†´JÜ?«¨D@òo'?íqAt¿p? ÿ›Ëó?™4쨕&?Šj?ˆöã?¬SåÜŒq?œi«p?ì3NÂ?©›sËj&X?qL±¿O[?s÷•'›–Ã?½PÄ~¾Ý?©¡SölñT?ïåªC,qð?i'å˜?®?U²TX]?R«]þñ1»?^ù%¦óÁN?c	âÆÅ×?ï¢2±û\¥?‰'™Y´¥"?hÈ!²ÑOÉ?hå%>–ÿ?AK£Îà?…&c=¨\I?îù®{²Ü?Œ½µW»'ß?Šø!ÞMÝì?}ž=ÀodC?"Nªy?†Oaù*‰þ?îþ&û'º??‰u}Ž(ÕÀ?_š"P	ú?S¦UÝ1¿Û?žAwV"/y?‰b|žwAGN3FGL J1024.1-3232@pãrà\̊@4Ðï 6kÍÀ8¡ÃPLH®À;uÝæЄ?ó•xÕ©À-@¦mV½@¦L A©n¿äŠ«Áå=¿çž9='A§¿çŒ¶@],¿æ::×þjeAGNfsrq?ïùÈ8`?C#?J¬Qä?='×J…æ5?8¥Fô6S?9ÌøÖLƒE?5jÀººa?ï¦Iõ[P"?ˆ	X3ìÃB?páÔ?³Á?n÷ð‹®e?{ù1.si?"ÜO"‡Q^?îè/¿¾Ïè?'g`c!u?5_TÆ£4?ˆûk©?"_Xbêl?‰•ÑçR"é?ï›_qLù?†Ï3<?ß?bª£fž?f?á"G†»?"}zɸ¨?…Ô´"ö?ïý;}_/?+-@Ÿ"DÅ?+E•¨I½ë?$™|›#þ@?!• (ˆ?MþMm"?ïÛ.žV?põ·59?]%Râ0z\?WUÓI¨:}?f?NŽ³Ž?k~´ÎÄ¿?ïHÈS@nÛ?Š¥ôî?hj?ƒìޅüt?zãÊÝaÚ?‰á¤òöÕ?…­0¯ˆ3å?ïë–|ÚÑ?b2ˆÓ?P—žI'Õ?BˆÀ"Ž~½?X;iÁÇV‡?`Þ(Ë=eAGN3FGL J1024.6-0718@ouÛߏG0@DB+ ?:¨À:Z÷xr¥À<J§Å¬G?ù	ùé-@5ò1
d?絫ºrF¿íqTsD‡?êÜiÔ¿èABah>¿ïÿ­µ/w<PSRPSR?¸Ñ‹cÐþÃ?ÆC<dN"?ì'eÝw?ǖ+W³+?ˆð¤ßä#?ïàÇ,Y7?©V¹ajf?À øJKu?ì}Tghøp?Æþò_"¡H?®Ô%r]ô?µðÉd	*P?ÏãÌ ] J?²Èm¾?ä¤íd"Kž?´»K¹‡¸?»üš£by?§ñ*{ÞÜ?À¨pñs?¾ž<6[²?ëœ&ÍÛPÚ?ÀnÈ,!?|Þzî4…×?†ð`\µÖ?­YÕ
¬ô'?ºLïk8?íŽá%ÒÖ?ÀŽƒíF%:?"‰YÆÊô?«ÔýÀ,!é?Áy±€ÚÊ«?̎ÔƸ­þ?éjƒpQ:Ÿ?Ð(ÑJ_õ‰?±¸}æW/?±¹Ô ÌUé?Øy"÷?¹3Kñç‹?á"tl
šG?¸ÖKmêþ·?¶æv›V¡ç?¤kzD¼2ü?Þ'aСåæ?ÃƕI…?à¶ý‡w$œ?ÃêJΧº¼?z¨ÈZ}1?ŠJÏê¶5PSR3FGL J1024.8+0105@ngààëgÃ@G$:`NqÀ9Ýë˕•(À;¹ÀI0Ëz?ïcV†Ê_	@
ª£¶~â@d±€9"¿à'…gÏ¿èåÍ-}¿ìK9ðø·H¿ãöÉï!áAGNbcu?ëR6¤_xê?Ák
ÿ§.q?±ÅÝz‡8?´kÞOØ»?³¨mb0ù?¸T#(™k?íTÞS²Û?¾ô:,ª5§?¬Ùú_t]?¶*šñþø~?¡Ñ õÁÿ?°ÔÚ§‹2?êŒ,¸è
ã?ª‹ÎÁÞ?´½ÍFîq¥? «æCÞ'?¶àÌð‡\Ã?¡­'É?áÏä°3?'vE½¶?Õášî?Ĭtœ¡Ñ?½7xbùZ±?¯uïN	«Ù?ì¿!÷Ý­×?Í-X±62?§2«\'ZÄ?½½1+àÈ?¬Û5)ßJÉ?Àƒ[ªΧ?ïSø*µÈ?ž
훧Ðd?ˆY…ÈÐj›?"l"ǵ›4?'¨o·QG<?'7~؉U?í·N·YYI?™_@€™Z"?¢ˆÞ
ügÑ?',>áâêŽ?¢6}Iê ?·%×¼%F?ê¾x i?­DyÈíú?ÀÿsÞI!?ª
Yã? ¦~ÂCU?'®O2AGN3FGL J1025.1+2333@jZe>‰©@LoüõŠÀ:"ÜޓÀ;ã÷YhQ"¿ºþãA@ÉAÂUP@™ †¿åÞ¡ï\!r¿ìqz@¸Ø¿­xÕ~]d¿ì{¡ß8_BAGNbll?ï•)L¡ç?I—Ÿjl?\B«¨?\G~à?‡6à/ãÄ÷?Ž
	>GWe?îâà†#VX?žkkÑ
?"Ê̐"•Ü?"Òzóñg?²Eg1JL?xy%1?í3ÊD(Æ?? äo¾šS*?£ºòzss?'¥•'§PÊ?©· ËÕ˜?˜^¤f]E?î€RN'›_?¡G›ñžÏu?ˆ§VÍj?¦|>–"?¡õV­–¸?}^ËH†?ï²cà$B€?H	^AŒ?Vlë±V‰+?Xß2ó+²?€™jx-‰?
®ÀÙ_¾?ïœ÷^¾Õ?Šà)î2o‹?{â$ó ì?ƒßw,…ç¯?u¡ÀbØÓ?uü^^2ê?îN²×?"ÝC¢"À?šúâÝûáG?‹a"ÂÌâ?›BzlæYÒ??
xO«?ï§86¹`Å?y_·8Û{?tÙ/ò7Ä?j´ÐÅht?wŠ´­¨æ…?q"o,4p³AGN3FGL J1026.4-8542@r®€{»bÀ7¥pà<ìÀ9Q½‹ç)À;}«Âßä¿åtªÊ¢Ò@
×á°ß†c@\à*͉¿å€4$Â#ž¿âB÷ÑÕ¿Ù[$_AY¿Ý»‰-±éAGNbll?ï•Ö&ÎÝ?¥¿;èÚ´?T*ëba?X1>mLTZ?œê£[ì
P?¥gj½ "?ï&ÙBÑáµ?žõ4…{|?xõ¾gY­?€w†7Ôºý?"ç•øe±ÿ?š™`v|"?íέ:hå$?™•v!F+?•¶ƒ`ýXÌ?'ª©@f†¢?¨9ꤧ~Z?"ÌÒè+S?í"SMK/?œT𿒞ö?^hˆ¢Ið%?\[]ÿ"?²ãÅ›Š?œ	ÐÜÌ«?礪\~d?¢È7‹¹Zu?O¢Ô:\µ?mšÙÎP¥?"'<Áãuí?¡G¼ÐQýÔ?ï½óM˜Ý??È0Y?`€AîÕ{?W˃úˆ‹A?xÆ8ŽßÒÉ?{çeû¢?ï'B¢øú?…é
ƒJÚ?"¿rî aS?s<W?ž"Û?·ò ù‡±?€Š ݟµ?ïi
¼šê@?xI‹Ê±%?I$c3«­?;ì~%ên?'%Y•mq?wÀNd"
®AGN3FGL J1026.5+7423@`ØÑ Äe@Cœ¦ßÓ9ÎÀ:Nd!À;ˆºô]4Ž¿Ý·P‡4šÅ@´A€}é»@•= t.¿èΙ«7¿ìó?ôüZž¿Ä
‰d‡¿çÍRh؆"AGNbcu?ïïHga?_uËSùÊ?2ï[o¯É?/ÃBX"Ï?\³lˆzF?]×Á"'ÉV?ïgl~a"?«³÷5{ï?z®Kù9?ƒä?£v¾?ˆÍº¬v˜?©=æ+ÍÌ?î~³àJ`ª?'^ôŒlP?Šîaæݖµ?{¸…Xt)U?¡Y)…+¯?ŠÁMÙî?îs¸›´ÉB?œÞdµóR¯?b4ä@c?aÊÞÓæ??§¡(œzY?œJ çTƒ'?ïùöì@Û?G›^ù\8?"1ú-êV?î(Œô8?C›5³
±‹?E.¸!`?ïÖîòšz?môøv߀?bÜ-<¢l?\¡'»Î3?f4ßäŒF?d˜Uî¿Pæ?ïkån"B?y´®åZ‰ ?yPx©º?gdgYê¥Ð?ˆƒ|$Rj'?s¶V"]ˆþ?ï£ÔeÈ[Ï?u"÷ÑO'?W]€ùäÐ?Jsº"?"6hÕ&?s zóáð"AGN3FGL J1026.9-1750@pNÔ@(äü@@\ßÔçNÀ8Ÿ–/ÍËÀ;,WvßZ?߶ÞÓ#lÛ@}ÙõI?þ·ÖÁañ¿à]ý<½[ҿ܀¯õó¾¿Ý!+‰E¹s¿Ùo¸ÕOAGNbll?ïüE€	G?4óþŸP:?$õõPT?Wû3¯?3YBœ?0À—…äàÃ?ï¯ä1z?ƒ55…?os
/$£?mC©#ڍ›?xTb?&¼Æ?~ÊšSãã?ïOÙ¾ðº?"¨J–ºÆ?'ý"?{9ª—(D?‰r«Îbj?{¸S
'
?ï_X@³Ï?…Á¹ÎaZ5?I#R'mb?J¥kŽp?"Sºlkñ½?…"X]p;?ïþ§y<h!?Bžâñ~?yù÷"y?é"·?–Ú"ÖB?Bìͤ?ïã¦ÅE?e†v/"â½?Xq'›û×þ?S8ÃHE:[?` q¬u?_ cÔc¬?ï¡ôÓÀ˦?t±ÛW´?w]2‡¨?py'²¼?wó8Õ@â?f2«?àì?ï×üdPGÒ?`ÌDáaQz?A6Ӓ±[?1ºÎþù)?qàÇݗz?`Lh~׸AGN3FGL J1027.0+0609@m·±~þá@Hç3çüÔÀ:\øÍØÀ;ÓÐJ/Îû?×°ý˜G@¤H"Xšv@¿¯ß/j¿ïòýý¶?ÍHਿ犋¸k¨¿Ðqþ4£Ë¢AGNbll?ïòR¥¿AÊ?TúTË+ˆ?Pr Ê8g?P¤'†?EÑ0¨Öãƒ?BåsÁ‰?ï‹,lÖ©+?"ð§W?|g«JEg?†C±š<7Ü?~Ue(?"Óü:$se?ï
Z‡œ'O?†Y"ýÅÁ?Œù'‰¢.'?q¼½Ùg?¯ËSþ+?w(t¶³ÍL?îËڞiœ?›À¨,?•ä¼8ž?—^4â·z?Ÿï³§mà?‰…'…æúÅ?ïúçIЮ"?=ýŒîW?4'ı"ˆQ?2°NY¹"j?43ìGIMâ?/ð"Á˜'n?ïÛsý'T?s¢;¿ùɓ?a~ž<%Ö?eùɝÖà?c
d}¿.»?jµ{'m?Ž*òê?t&)Q¶k?~
7E›{€?j45Ði‹?~Æ—;4?gäeÑ[Hñ?ïÄ \k?rXÍ~%o?q\ë{¬#?e¯Jš™N?hÇ&¯ý-?gÆ'öÒ,AGN3FGL J1027.7+6316@b6@ Ç@G€8_ÂÞ7À:s­]èÀ<)Ó8 Ù¿Ü­öaµkv@…¤ƒWÛ?ÿïkˆ±j¿ë¹²œR¿ØØ>ÚJ'°¿Õس#È ¿äÑ©u¯¯†AGNbll?ïñ°¡Èè?^‡R–2Ê?P›f¼ÁÍ?V"»wO˜Ë?H]\:Š3?HíE&äØb?ï*Óyþãd?›¿³l{?ŠðÓÂSYì?ŽxìÚX)?ŠZMÄÓ?'(GvpÀ?殺
Ï?'mPb…e?†ÜÔt?v¼ÒBÂ?'}S"Ó?zzzô€®†?îéíMºŒÈ?'4·Rù2m?…ØYvR'€?€´nÏë?—Ö)†¥åÇ?[CŠ¨ÁÔ?ïúû§^[ß??Y¢4æªÁ?/Ë"Y±?31 ~³ç?8=Al´Q?4›^t@'Å?ï˟¶Ç°a?ub"¨?jZÿlªc?esę\½Ý?jJùdi?mfcî¿¡?ï%)¸¾«?pJÌׇ"?{"Š(Fø?d;doÂ5ê?'3ëXç"?gß\äŠî+?ïÅ(sfª?kY¼¼ÜT?h~äØvj?WZ¼w\³?q,T¼<?eMÙé÷;AGN3FGL J1028.0+1829@k}ì_9K{@Kýfàé´À:_—+*P6À;ìRb£cG¿ù÷aüt	@Ǚ³oق@ä]_šÊ¿Öž?ý'3¿è;h³Ÿ_¿ßåå¼þy¿ÕÚÊPñŠAGNbcu?ïè}ñƒ¡œ?f£…ÌJUk?9/åe"'?7ËÒ!?8^?d\æiÑ_?fxøj܁?ï¾è…-ô?†hSòž'?mÌi®zd?'>Í:óÖX?q¥|_LÅÄ?s}åLJ?îÆF90‰q?‹Õ9jËI?ýË(z ?€^âí­8y?—/;~%À?'{ã>üc?ïÕ…/C?p$ÒXŽ?C\ʾ?p ¥$
­?uñ,œxï?pi*!üÓõ?ï÷ðK	Ç?Q"0ÊÏÑÍ?+Æ.¸m¥?-#
¼ë—z?LƲ½ë%-?PpºgêÕ?ï髕D C?bŸzÎ#?TÇZÁÈZ?S
J€?Xf5A=?W<ªžƒG ?ïkG°²~²?€ÄEm‰!¨?¨*DæÓ£?xïJß O?ƒ…éž÷ŸÝ?sàWÅÄé?ïùÂ<Œ3'?DJ"Wsº>ï\ÖE鴉>ç?¼7¿?Hy™v£‹?D.e¾úãAGN3FGL J1028.4-5819@qÑÆø¿ßµÿÿ˜ìÀ6ØSéŒ À9Ï´ÂêÌ@yuòËd@1<¸íó@®†‡C*Í¿É#»j"‹|¿á̈&œ'¿åé7ðS²¿ëÂθŸOPSRPSR?SUÚß«gõ?U¡&-ù§?ì>4|´\?ÂBìioŸ?½ÂníüûÇ?Â5f͔s??	‰óéa?sü·$\¿=?éî½$¹í?¸TgˆÀÒo?È5~çç…`?¸aä§|4?'»á'ã4?
†Š\A?çã̗Œ'å?ºó¥árî?Î9Qoß6?¹0Ž:±Oð?aÇ"Ì-?_&âïƒC?ê¼A3slV?±¢‰7éÕ?Äʺ¿À0?±x9üâ¤?`Ô*®#Ã?p…¥('ç?ìPjoÏ4 ?Ä"GÈÁz^?¼ö4''?Ãøhd ò?E2tòc¼?ftO¢õvÜ?ê":Ÿ´è?°åÑN`¿?ÅÙãC!?°í·…'Î?–J'íôR?"yBô?çZ>>Bõ?´èތb?ÏÍÆ'RA?³Þ³'•Í?_vl¯Ì¦?V¤{¾s?ëÛÿ§Œî³?¦Ý¦ûâ!
?ÀQD=z=?¦¬‹ñÆPSR3FGL J1028.5-0235@oN ‰ãC@FD!?ë¨ZÀ:^ÖÒ	L°À;՞¢ŸÓ¿Ü=ȋR6·@½;¾	;@9Nª¿àÛµ7QGh¿çü4Œ'7†¿áðzŸß¿çp¹Ô«*AGNfsrq?ïý…Ž
¹?,[4ëîŒ?zÖZ;Ú!?²a¤³Žž?,é±q>!?')GcT?ï­¶ú}Š?ˆzjgB}€?sÒí!Oá¸?ƒK¬HÙÿ?uQ•…´?xËåâî…X?ï9tíàA?"uPݽ´?'
*êÿÀ?w¦Á£`†??˜™›E`õ?{Adqj6?ï±IÛÚö?wÜUÖÌ?I\B1Ru?Cq¥xÊ?''gÒg
?vžã:æpŽ?ïþ€Qƒ?X(ùïÖ?¯¢ÖÆ Ç>ý–ãÔŧ8?#'1¨oÏ?Xè*Bi?ïãII†B
?dËA-Ò¸?Ya¥›Ëò?Tçߟ…?`+Blï¿?\Oˆ÷ k?ï®íSނ
?lãUî}°?n×êøZéá?]"Gë#Ó?y`«îÞ(?e+Þ£ät'?ïðϚÿ?T\AÛÕÆÌ?1·ž
÷DÍ?!Hò.ºú?Yòâx—(Ä?SR "X	AGN3FGL J1030.4-2030@pz-••@?eþßnÀ9¤ºB†MÀ;~o09ƒ¯¿µ*ÍóŽ8°@´ìL™á"?þ;bŸ1‰¿ã
]Nd¼î¿àÕAêáÇ¿Î?©˜5Á¿àkÎZXAGNbcu?ï÷žI׏s?B[÷Ëq¹œ?<KÌ;Û¦Z?1•Ê Ÿ?C`ñ±Eé¥?:–è£Å"È?ï^_±ÁY?†³g\@ÙË?t}]¤"?pî!Ööc¢?|ÓrzB?ƒ´Õ»_?ïTäì±Í ?~üWu¥þ?~"]€b]½?ië>òU?‹"–#Ù©?w
@É2¸?îã8ñ°~Z?8½d{µ?aT*†\Â?^`áXS_ð? »«¢'­?¨Rkž
ç?ïüÒYå¶?-C<Xë?+øÉ×íÖ?QÐâ'>~?1'ðÌÿÔì?%LŒ¿¿­?ïܹ"»¹?kZÔõÁµ?_¸ìŠø*?Tœ¼§!T×?cjg+Ê
?f›Ì Ž›?ï§ÌJ¤q—?mïÙÀõÚ?sEނÁ	?cìIþE|¡?y"ð@³?d9`ÄDù¾?O'
ë?k½^`¯?UªBK'Ž?C:âvôˉ?|Œ—Œ¨â8?iÛZLjR'AGN3FGL J1031.2+5053@d.%¿­@K7èÀHZÀ94
ƒvA¦À;UÊÆbP¿ò–i¹W$@áë#$j?ûHŠàï§?²ïâ{ŠºÚ¿âÝoFVH¿ÒñŽÈá¿Ífl_hŠAGNbll?ïöÈû~]?PFOÚ-¿?<aÍ4?7n"ÐĘ?I'*£»[3?M[¯ž~³Í?ï¿Ž@[K?€»nXµ½?jp® |?q5>ÇÚ(d?sEa''ÂO?wð†v5k9?îôà$ #?‹Q½·"?Œ­FÓ+¿)?úØÆћI?"&`‰O
?'‰®rú2‰?îõS`)í?±æÖhv?6™d°* ?;F6³ž? ~¦Î0[/?'@£¢ö©?ïøÓtöeç?Bö‹]=L?;4ýíï?4·•O'pŠ?>0GՆv©?:ILdçâ?ïæÓÜêó?g.ãs|?V•¸.÷6?T:¼uÛß?[
dC?aµ¢F?ïp¡À{þ?G[ƒ¾L?áK³'wM?uÑ¢\|Pà?úËç](?p¼)Yr9'?ïþL<ª¼?lëãb˜U?è¨õ—)?vOÄ'~?}µ7R§?¾?lÓ°™ôaAGN3FGL J1031.6+6021@b"àç6@H›¿çáüÀ95?VW$ªÀ;UøZ?Ç% þä@	1í]ç@	?n)ÿ¿è˜ùX›øo¿çpØæi3©¿ÞµÕ
|Ú
¿í/ö‡,AGNfsrq?ïùúWýön?D^@'©ÈA?;R_¶?<Zßî"R?5'ï!'ˆ?4ôÃV{q?ï›G{Oé?‹.¯>Q?wéÅ¿‡?ƒ'"Šå5t?{UÌo?¸?€:ÂS¹ó?îHş9Ÿ?›Éú…MÏo?£uÏ?wê-–ø;? 	æîíü ?"æ~Ùâ¥u?îj&EJH4?š.ÍU°L?téi¶?r/<	TÂ?¦Û~{½?˜´;ÀÒ@ö?ïùàïÍ
"?D¸6S?B‰ºž_ó¤?Aìœv¬=?'Ê´í5X?!lN4=P/?ïß-mãf?i™ÔêŠó?_j°i"1?Ygµ†ã1?aVsWý?aà6ŠìÈ?îɘ0Oî?'­eJ¹&?"˜
ÓRLÿ?†ŒÂNX?'4ñÁ|KP?‰ì¹ƒAÓ?ï'ö‡'Éj?tåµ9ÿÉX?fÝÁـÂ?WŸÃ푦¤?…ÊíÌ7»?shÍÐT*AGN3FGL J1032.5+6623@a»/ÀL‹Ê@F¦>ÿðÈÀ:ìÕy(
À<MiŠÞô¿Çæ²üìû@A'Ž³6¤@2o¿¨Í¿êÚԊ¹àj¿ÛâîwAý¿åþR—¿ÝÀÖw¤	AGNbll?ï¥F©Éô?=çÌjlÔ?…TlѪü?Û«˜çÆb?EžŽ·w\¬?F`â·2?ï¢?î,˜å?‹À½òTËÓ?w@¬'ú~ñ?"G¾†ìs?wŸ\pÖL?~ځD{îƒ?íÂrÀ*Á¹?¢ £ylS?¬Wdl›r?¡º¼cyö1?ò`-‡æ?õ(Ö0?ï¬! ÛúŠ?{k×N܋?iƒ9z‰ª?gÓ·¹Fˆ}?}-'ø§.u?vž	΅?ïÉÄñ¥ãï?›îôpÓóJ?yy¢ ÔÒ?›ß´RyìÍ?:>I8é°Ê?VbnE¦P?ïáÈÏ^™á?j['²ö?[`×w÷§?WdçAÅ)?`†Ä§ÿ«Ï?c`¾XV3?îb¤Í6w?ÞVV£?¦&—³)Qw?[Õ¾_æ?}y@˜Xò?sy¶\mm?ïòÖZÙÚ?Wä+ÜÒQe?DSŠÅzC?7¼ÅÐ|Q?P)"½Ú{?S£§ï°˜AGN3FGL J1032.7+3735@g
Âß
A1@M‡9á£À9A§~^ª°À;ʒ~e'¿í!ìè0"@Rk~SB@™÷?':¿äìðgAéÁ¿å*<éâ©¥¿âX<'ß©/¿ä²T²ERAGNbll?ïjìƒ(?Œ²͗Sí?pѵ'LP?nq!¨ã¸È?ŒÜ"/sÃÄ?ˆ¶ù<F¡2?ïBåljZÌ?¢røHg?‡
'ñˆ¼?•xF'Õgø?ˆ;ü9ß»5?'íò=Gÿ¶?í"rn:"ï?¨£óp¹?˜øÞö…o?‰"šÏ'²¡?ª<i¤ÊªR?—YeT¡¨?îFÇ
|@ÿ?¡ƒÇ¡È?‡
~øìUø?†õÒl®[?¥Ð/šڌ?ŸE´oQÕ1?ïÞYeˆ+C?j»…)ݍ|?S×´™'—[?OÓ©Mµ?gºÀС+?fbþÒÙV?ïÍWã'z?…S/€_ܖ?iAù±Éœ…?}¸¾3=*?if#2"©±?r±ïŒ8?ï#~-¢?‡Ü<kyä?‡1ûRÏÎ?{óùÕ{?îv™¬?!SÞãžu?ï»Ky¿ÎP?tˆg0¨vÒ?T:Ô|Ïu?Níá戹?}K¼q(ïà?sŒtèÁmAGN3FGL J1033.2+4116@f+zß.Ï @M2R¿ÀtÐÀ8áî¯u£ñÀ;·uª§?ÖLž?Vé,@à Áìt@'Ð pË¿ßa£½‰ä¿çB‡ÜOC¿à<%ÿ²Áø¿ì#ٍiNgAGNfsrq?ïôƒ.Äd?WW³iP0?NÓyò"Ì>?Uêlb"O ?>@	/?7¬G²ßàê?ï4X/ӝ?";vÅüp?‹BGFgLÓ?‡Ä÷í"?‡§¬ÄÔÚ?‡ÌÇl±FC?î±TLn©½?"²púãÐ?˜[£|):?Ô·«<)2?'yÓ_öÑ&?…#Ÿ¥ò‰?îÅQ116•?›ˆ«îWwe?Ž?'™]Dæ?…àó+x'1?˜6Fr¼ð?—œM9Tñ…?ïâ;i7§?¡œï([-?l䦜Ý'?¡õœî›?*Ë&'~æ²?*­ô'Mm.?ﴕ.-˜r?yŽÚªQ:?sòSÐOÎË?nÎEª"§?qÃýgC?p´áÃ?ï2}_U?d.l"ÀÖ?6­ç"Å?†ÍxæyO?'ób_´7?zipI"º"?ïÁÅ|Vé?tYS@_e?nØ= £_Õ?`L²ÑàÛ?obÁV§¢?pðaégöAGN3FGL J1033.8+6051@bxæÿ}ú@HŒö@c^À7Ç9k[˜­À:Ñ«ì'tº?úy4I]Áý@æ~ZÎؖ?ÿļ'ÂåÿÙ蘙®+;¿âÛÆT¸"¿ä qFŒ¿èjó®AGNFSRQ?ïðÙûo³¨?`´
ãxªË?IóR£Á¢?SƒîXŽ?QR|8²'t?X±e%é/™?ïÁD¨rò³?†¨%2'®?nØxÿԌ¹?'ÖÑ\ÐLË?oâÞµ7Ý?rOþv=?í	¾`›?¥ïï¥d?¨pBÒf?›à[AfŸ?¦ÿ¼ô;?Ÿ«Ûiy£?ïåý³¨=?mï±³Ö®?,‹²D¾Ô?D…%°Â7?h9›ëK¡?m]¥uŽƒ+?ïß
Ÿ®d5? œ÷¯êâä??'Ìçk)'?;ÏpÌMfÐ?m§æ@Ã? ™ÙQÜ'?ïêMð\8?eì仝!Ô?RŒÍK¬_?Sh%‰v"µ?XÙT̀
?^䙟gÌ?í³t;'%­?£¶°—í/?¤qe¢5
m?œBÈZ)õ¥? WV¡HûÍ?—‹5œ§½Š?ïúV	âæ?Où¬§Õ?""gÜ!¤(?0'ÁK^´Þ?BÂte[w?L8KÞzÛ¸AGN3FGL J1035.2+5545@c?ʞõ#-@J/xßå®EÀ:*ôœõn­À;ñ<¼HñÀK|7³ög@Þ/â+Y@‹õ €"Ž¿èe~Ñ[¿¿éöíO×·?¿é«k¿îøË1}bAGNbcu?ïî‰Ëì¨?lƒ‡TŒ»
?5Âõ³";?B">€bZ_?]}9!@åÌ?k5͉Žž9?ï´u~˜rŽ?wETE™?p4"$¯?q²\^Ý?u­—l(?xÙ̖ÇYR?î_˜iBä¬?™g˜4Ö?'XÔKý?†["‰\͛? ÚDZfÃ?–î?
\	?ïÇVÛZ?~I¯Ñf'?@6"Žú5\?R¸²Ô  1?zMçÁø?|ÿ艒ú'?ïóqPǐ?g¼¹°ð‹3?;èR›ö5?@ehy|aJ?R#J+Î0?f'Ï@0?ïç™{‰?nLç«h?YÏz3EO\?hI'6íq?WýS¡&Â?Yîø¦wr?îb
5&í?œd,¥O…N?•Ün-ï¢F?'!á½yç…?âK)í?—ùÍýG–?ïøÿ±Ñt?SÃ*FÛs>òŸŠl?›½¾Ó"'?O#Î[vê?Sjþ*Ü°AAGN3FGL J1036.0-8317@r®½_ÜßjÀ5O_¹£ûÀ9àG­=»LÀ;®ygÊêt?ê÷6õé@
ùpò[|¨@¤H©hš¿«_QÒ¹(‰¿æL!·hj*¿æö}‡-Ì¿ïÿ-zYPSRpsr?êÈyËñ??½5ÌîÒþ?®Ú_Õ¥#ì?°äûÇhF?ºO½;ה?µ*ÞÁe\?Ø`å…LÒä?Ė,‡rzœ?Ø{ÉÌ´›u?᤼¹5?ÎF¡^"äË?À†µ€ØÙ?è¢UÏô?²Uðäüeä?³Ìjý$?«d@i¤Þ?ºcT…Š»R?¢~Y½ÄC?ØX‡z! ?³×8¤ãÙí?Ú¾¦GÁ¤i?·æÇÁªlÁ?ÉѤ|:|í?¯Éé"dÄ?í9Z¼[‡Ý?À|>ٞ[9? aÒi*!?®- ց"ä?¬Sòjr
?´ðÓŸ`y?æZ'‡^P?Àdä¹±?ÈË@Ù?µ°ÿ̝_É?½ØïMˆÒ?³\@9)b?ìãîb¯ß?£¨È¬…?´Õ+ûb_¼?œÚvèñnã?¦i#Bœ?'ˆ#ªž?æ}E¤K?§€™ë¿zV?ÊùoƒŠ?¤Qf:v½Y?¶#®1HzØ? !ïB\_ÁMIXED3FGL J1037.0-2934@pî¼ßï¿@@8Ïà0VàÀ9¢<PgÀ;‡vG…?ï­Ýò ,A@δMÏì'@½æ¿Þ}ºüüщ¿èGL'!L£¿äŒgv©!¿ïÿ =Z~AGNfsrq?ïõôîvb)?LG‹aށ?F.ߣˆGw?EîA{h€é?AýeÆêÚk?;×j-Çîª?í¸;ZO#?©ŠÕÐdX†?¤$_!;?™ì43GÜâ? `+[Dì'?¤'Þ?î!O¨ß²®?œ.QX)1?¡‰=TÞÏ?'Šu±ªSó?˜Äg¨±?ŽÜ›´Âc?êñ{a?ª¯Tœ…?µ³y<¿¿?¤!'ú½Bc?²Á~–ÃW?¢'Mbóå÷?ïúÈœT??!to†§?>ÜjFž~?8š÷üíDh?0mPGÃNV?*C.»ú~S?ïØ~øP?'Êá¯ҋ?"³
Ô¦R?†è3o>j?ˆ¬™ÛÆ«D?ˆ×7X³;?îû¶¼Ì?Š‡~¹Þf?"ùêíDš?'5VUP?‡|º27Ø?yÔ­‹ÒÓ??íþ;
‹óƒ?',bO#«`?§X';§ ?Š¾7Û$³?'‡{ÐT?ƒ›®'g/ÁAGN3FGL J1037.4-3742@q9Ê?‰'Ë@1òŽ AS‡À:*®í¾´ÜÀ;ÅÌðÞúÍ?ÕêêÞÊj@ä4i>÷@
îßòŒ¿èb^<¿æ/Y^ëô¿ë'lkZŽc¿ïÿ9M(¨AGNfsrq?ïµ¼jT½?i'#^k?y%Þ*?|Z¸§4?gùsúó®'?i"øDv.â?áîÛÇÞÈÅ?ͯÀWH'>?ÔÓÃOå4?Çv'Ž7»?À8éYåƒ?À°•§¥(¢?ë÷Òyßêâ?£xýköÕ&?®f¤Ýߺ?–òSêÄÍ?±"í ?›Œ[W]˜?Û5ˇ ?¼S®Ó½Ö?Ü̝'w'\?Àœ™ëÆYŽ?¿ö[š
:"?¬f¤Y#"h?ï׌ŒÉ?rqÁá{Î_?lȜ0ã¦?oA2êSì?YÚC¿Åé?V8±¾/?ë»#LéÆ5?º[r¨¥6l?¶Œ4š%*"?±nBÌÚîá?§5aü=`…?¬FÖ{%?íÚª5Yd?"Ky¿ÎPt?£dΓyن?‰0tÍ(à?ö-'a i?‡\ŽðJ	Ì?é°i;'§?¨å1&ü^¯?Ök‡?§>4þkS¬?¨ë<q-;?•"v`ž?5MIXED3FGL J1037.5-2821@päo€Uûµ@9☠uUíÀ93Ád¹½üÀ;€C_?ÒïñŒA9@Õ Û,a@ñºÃ.¾¿æ8÷׬=¥¿åáJ‡°Œ¿é®÷!F¿ä"\@?-AGNfsrq?ïüS?5Z"ë÷‡?0Öaq½[[?,ý	ۃ\Ñ?,±Wie×x?+‹ZXûþ%?ïi²ï‰˜Î?™ú²3%?|U"×k½b?y§)Ú¢?‡hª¬¿Ñ?•Í¦ZúÍ?ïF X$¯7?€›GÒN,c?¼ªK଒?r\$^P7¼?Œ›?ªó…µ?x=ÑÿÌ^?îhƒ.ž#?—FÓ2ža?‡F	KC¥e?€A^;îòR?£¦J¿ÝIH?•PnA!"?ïýîž6iý?$ėC?$J¾8O,?G­»Ž—?–¹	Rü?õZ‡ì‡!?ïΒ5æۆ?w¿Ïʜ?dtMNþ]?[MØ'ÚF«?lù}TÜ
?s@O:ÎO?ï %Ŕý±?t7¥¸%ÀÃ?vyU‰ýÍÔ?nQ…)?ysÇÉýq?gÿÈPu?ïª
ï·?tڙÁ$…?iÚï\¿'®?U•Ãâ¤`?~•æ`?r¶ '…²‰AGN3FGL J1037.5+5711@bùŸ˜=@Iáü`8NüÀ8<ÃÕ­FÀ:èâï?õ.HËùp@¡½Gɘ:?ù!†â-\¿ÓS'¼Ä¿Ü,+³sE®¿Ù[žÔA
¿Þë·V¡öAGNbll?ï÷ª%ÁI?^±QaŸ=?,lä•p¬?1"o®ž|?JUdÆwL?[Qš°§ž†?ï"CÑ9Þ?Š"LÙïÂ?wôÅüÜY'?yðHú4"?~i·"Wkœ?…A¢ÔÚ!?í»¦öGp?¢hjèû?Ÿ_ʗ¨ã?•ë9º u?¤•¹§`i"?™¯çkcÅ?íc‹+¨á?¤²ïZZ-b?‡YȲܗ¸?"¾~9ó•?±üºŽ!d€?¤KÒ$EFÁ?ïüïwF³n?0èJ,s?"Rû3_?Jj-ŒZ=?.µŽqÄ›?(tA~g?ïÒåå™ï¢?tOHi©z?dpܤ9ê?`#R/È?hª­(³?p·êÎþž?î¬Ê ;°?—qB"ãÒ?•ÅÐh¿…\?>õå?" ì¾š?Kœ'úh3?îðªô+'?†ÆÑtÍŠ?‰æYzj‹V?w,ÅŁ?"÷tÁ;?ƒ"—Ø ~ßAGN3FGL J1038.9-5311@q¼ M@·o?ÓՀÀ8-¿¸èzÀ;)iϧr ?úÆbã$''@F5‰ÏÍ@#Qv?Lq¿ã¤˜";¿è@;ªóV¿ë'ÞFz}¿ïþè"IŒwAGNbcu?ï'zÐUÃ?ƒß¢ºò9?|›Šø#-?xµ°´j!?z×·Ÿ±'(?{ªúÔïÉc?îuÿRÿè?°&r&*d—?wô®+a®¢?|ŠÃ*Ë$h?¥¡qGs¢?®¢¥Î.—Z?ìv¶ânŽm?¥póT˜U?°¨¾ÇóÁ{? ¡dÖ?§CF›áA?˜›"¢o4?ïÁð'šÎ£?'HvõSvn?[‰•Kö]?nÿ#"Oû?x ‰ËåØø?€s­üð?ïÁ·ÑÂØ?š
Ù\Y™?w¨»Ì҈?™ðÝù¾?`$ÝI瓙?`U‡¡jƒ?ï{l苚(?œ—µ°ÿÑW?e$AŸê7?l‹0šYK?‹ÛÁÖPcƒ?™ªr®b?íqtÎâ?¡þ±õP½?©.b{
½g?™è5Øv?Ÿt¸ÊÈvã?"¡BÍ¿?ïñËtæt?bÖ
U
˜ê?GÈö¬ëO½?Wì3uEx?P"›3|U?X7<²VâŒAGN3FGL J1040.4+0615@nXà†8@JE»üÊÀ8Ñ:6\³_À;x§P;¶?éq‰žò@OŒ¼çQˆ@ÏgÀƒ"H¿áø~«E'Z¿ãõ1Tƒ1p¿á÷,̑é¿èÑ2uÚAGNbcu?ïñZe³g?'ªpO ¬?;²VG–ß?<€âÔ2Ǻ?V^ qì€Ã?'®äñð?ï{0Ázˆ?ŠEPF]j?€@ѽ0§?{éfbîãQ?2ŽÊìùl?ƒ÷Øièä?ïXu/e?'o.w¿?€jãÑ'?t@œ¦áû?‰wЭ=K¡?wô'rsY¦?îlTár?— 'טj?'>îÎ
½?'9{Ðq¤2? :"esÛ?"ƒ -édŒ?ïü¬9qU?3ÜF@«yL?/ؽªLô?-1©ª©â?%eÓ]É£µ?(óÝemP×?ïËXp¯j'?qP]oà?j¨ƒ/°t?cð"¨7"?iÿ«Š?hlŠÞ¬›?ï«Øe?r'«'?qr3ɐ@?^n'õ†?x¡ÊŒ ø·?p`J§Eå?ïÁî™È‹?x֟'…Ò~?}Á­ë9b?erM%}ã?yۇþµ?t|SQ$AGN3FGL J1040.8+1342@lÄHS'^@L]⟜èÙÀ:¦–À¡E`À;×Û©¢f?Þ¸4r@–`Þg)?ü(ôÀÜ©?íó™Úç¿îö'LdÌ?ë@"!'÷¿¿Þ «ˆìAGNbcu?ïé_Øù?q÷õ2Z:?Dq^!Sx×?fXÙÀ?a"–§¼g?iª¡¡ÌS?ï˜ÎB˜«Þ?‡iø)7ö?xy²ù.!?}´š¡}B?{+žÿ1?|ø]ËSx?îjL•ëöD?–tÙÆ°S?…;@àÕIF?tâu¶|‡?¤fh/bp?•U}8y"÷?îdÈÇã±?²Ùø×Åx?ny\­íóë?"+îÙ,¦?§Ëݳ€Éµ?²,-ŽO?ïjÓ´ƒ»ó?½ÆL·àùÍ?'ŠJèEÀ?½Î
ÿòéí?Q³ìǍ–?UKùÂÂ?ïÓhŒLe?v]đ~ë?f"°ïú‹æ?jNJÛH5-?ft²à"?j"Ñ?¹"?ï0Dõ?‹òéß/º~?xô&uè?a§ôã°«¼?–2A
ùW?‹Wì¿Ë i?ï±W$÷Rª?…½âkrÿL?ké}ÆvÚ?r1öÙ£èX?y_®š<k¾?¬N‹~ýÐAGN3FGL J1040.9-1205@p<>_·¼@C͆_¡PÀ:_Ü#åHÀ;×m‹ô•i?Ù)EÝô6@s¨(}¢˜@ÚßVø4¿ì	uéªíÄ¿¹e'»ež¿á`!œn¿åÞµ'ƒSAGNbcu?ïú©ãO?:ÐB{ø?7/{$a±š?2£'­
ôß?3k‹_ò?,.Ðyz
?ïPª†•Ÿ©?§ÆWœ+ì®?ƒ/¸ŽïÍ?Œã6À³?ˆ¦X§ˆ…û?¢OrÜzñŒ?ïX¯ŽDô?ƒˆT°Úö€?""•ñŒQ_?~H9?Ú?…±†zv÷U?sRƟ¬Æ,?îí·b¤²I?Ž¼ûvííæ?z
ªf<?€R­6°qr?'ŒÛ^¿?†;F¶CO?ïýºHä$?#É¥¦2Á¦?#7õT}%
?x?!#‡¿×?¯¥9=
µ?ïφeŠHn?rÖJ¢'Ñ?f‡ªqî°Ó?]TÔT•Øi?iñïèL{?n/a5ß¾Í?ï¬ÛîÜIË?wŸÓgï'?v^­^§Q?vC¥÷îà?s3[™{3?Y]"Ã4ŠY?ï´[Þo¡?oð̤ï?w]‹à??^1§GÐÌ?lé
ÉqHy?ežm<9.YAGN3FGL J1041.8+3901@fšž`=Wy@NGU?ÍuiÀ:Ò2Ò»#WÀ<]€
×Y?âUÁݧÝÌ@
÷œ{?ÿ'dÿ^'?ïþæj­ž¿ÍÀ…¿z²V¿æÙ«<%¿Ü×k\fÖAGNbll?ïÐ:ɐ¾e?yñù¾-³Ô?nn(uÁs?uû£àÆv?aW
ï1¶?cæ—5n?îIg:`f?´ðÁa0\ï?¡=¼Fi\??±Žô%'ó?"W ÐÉ? ØA8E'?íúX•å§\?œ:(Y‹B±? ê@Þ ?–kQiA?žàÔÁÔi?Œ´[+w?æÌL†Å?£ðóÑ&+?Ìò·Ü¿x?Ã8gqö‰×?±•¶[j`¦?«nÞn°˜×?ïòÏó?I¹?Y óáQÔµ?G¯~âš6?SŒ³'mUç?M³ïå݋?I7¼oP?ï‹5[_)å?˜5BD,±?,Â8g?É@ñÏË?{8)UQR?‡-3
Wœ?îéc²h-Í?
C›—?":N›É"•?‹ÃòL|õ?2v$'¥?6Èo—%ð?íäޘk
)?¡^Êmzk|?ªê~â©Åñ?›ý¦Èüê"?‹^^ùý?‰‡o vØyAGN3FGL J1042.0-0557@oֆÀ
¡©@F:ØÀ  À:kÃ
0j+À;ÎÃÍIÊN?òi´Ï€t@
Í."®×?ÿr?7£Z¿êﴈ³Bb¿èJWqMl'¿¦ÛnŒ`Ý!¿ßˆùiÊWAGNbcu?ï0EiãëÅ?žÜ•'"ï—?zNÑ§'?v—–jú?"c²IAQ)?›éžt?ïF³QÀUà?˜_×ÎUŒ?‡õpTÝÅ?lva5n?†]»>|^î?‹èÍш?ë*%È3'?ªe9qÔ?³!Ïu®æ? õà}O?³Jq¹?¢;[häùr?í¼ÐÝÊîH?«@¿dŽ²Ñ?˜3ڎ[–â?¥jŒI{©W?¨ߒì?¡M'B?ïx=Sr˜Ï?Îс3é‰?z"[×­?{"ú§<K¶?"®}—µ‡Å?ˆMž<˜A?ïɼąÅ?wxï›|õS?l\«ïŒ?kÅ!ZP^?j—+w÷a?m¤¾ÍFÎ?íZ¾tfѓ?¡"dmµ2?¦ä')Q•Æ?–¾<4el©?£o‡"°í
?–A|eðäs?îØ1¶!Ã?œˆEÎI*?›¢'\»Aà?™Ö'•»µñ?'¯jØan?zíUÙ¨^ÎAGN3FGL J1042.1-4126@qf1Ào@.cŠ '§À:˜PÀ;äcâ'§å¿û!tïÁ@b=OçÉ?ÿž/ÀâÞ²¿æÃڈ!L+¿èiòX]ËH?½ž‰`™üI¿åë®ïí
_AGNbcu?ïõ†Q¾8µ?Z;ø¹(B?`ÄB€l¶?0^¾u,u?SPǽt7?Y`ŠŸy?ïXÖs9??™›ïr.¿³?r ü'?'TéÂvª?]+
b?—'a´I
?ï?Nõ[Œ?†Éº<;?'ˆÑÞw?rñ£N)Ö?"NѺÁ^9?ƒoÖ?ïÆ;XúÊ?v‹#»ð&[?ïaØ{Ak?åÅ$ôE}?|²tÙ´"o?voV¨õó?ïü*ë2Šä?@èœÇ`Uû?7ýü;g?\	^å?9Úàæ°èŽ?@ivûŒ–?ïҙ±R¯?y^=ã9o"?Y¿"]œç ?U(—+0×?pCFX®\¿?vØó· R_?ï–;ns®¬?p0?&êã?s˜ý°P?`£ú©P‡1?€¥ Ó5¤Ù?hEˆQõún?ïõ'°€?Mōwå·â>õ½JŸ)A>õz¨WWà?T‡Y­%×?MuT¦ø¶AGN3FGL J1043.1+2407@jsˆ M@NÝÀ:SÀ9l5Qñd\À;²£á8k?å-ÇêB‡@"iÞ @ðO@Z
=¿ÙÿŸØwûº¿åSâì&Œå¿ä@½€­Ã¿åŠRĝÿ/AGNfsrq?ïÌT¢Ä?r²Î;:R\?r	}7ÿB?pUõó@`?_:•¡Ë*?Wa|Öm?îcÎ¥®¿Š?¥÷ñ¼æè¼?ž{ë"}? Ãg¶Wn?•
©_7?—8HiýÔê?î£|ّÏ?'»÷ï8¨*?'·nýÿ?"ÂÃ÷už¼?˜è"P¨].?‡8kLh~?éf¯ƒÞ?®WÚ0³],?½îÓnß?§ú€W[å?µ•÷bN?¤ Ã¾ˆ?ïñ¬Aß?ã?X]¤0+'ï?Týï¤$!?Uõ³U?h?AJûñ™7ä?98TZ[æ?ï†@º°@?L–1"Â?Œ|
¹Dc?ŠÉ˜ä¾ö?yßgƒÅ»l?{ÙÅó ‰?ïyÅÌ°û¿?zößr:?€X'îM³º?t³¥Û…›?5ùⳬ©?j*»Lí""?î0yÍÿÛK?Á¸Ýܳ'?£á»í¥ƒ?"Á軓[?'-Nb{¯«?…œ¿\ÚsAGN3FGL J1044.4+8058@`I¥Ò@AXe_Ö)mÀ9Àû¦ÔëÀ;\íbnŠ!?î3€FêÜ@™¬Ÿ°´é@"ÀŸAú¿ØEÛpBw
¿ë$¶-ׇD¿ê:` |!d¿ïü9®;VAGNfsrq?ïùQ؏Ε?E±dk37i?<ô¡6Ò?95W€ÇO?8|œ#&í?=ùŠsò?ïo	3k£?šuêQ'ÐÅ?n™*¿?4á#¿úa?µ¤£I+ÿ?"'íô]â?í–
õ?¢8Q|µ¸?­n®/ê?›{|-æì?¢‡ñ³qÑ?•n0À"?ꥀ=ä"e?°ûY.óÈ	?´}ô¢~Æ?§Sù¦ovù?¶´€ô<?¨®Ù-À½?ïúÙqdµü?B(&T"U?9Gt¦\:š?5½rônp?/Ùý¶?4Dñ¢k†Î?ï£`d\?'ƒø@m¬J?w-«VÔ?tÌB‰uˆ»?wp¢uÒg[?zK'zª©?î(à̉"?—ýJO Òó?£]lŒƒ!+?'yšÔ4Ó¥?")
\¸Qf?Š…s-/tH?î,ùlàJz?'ÂŒ²ƒu?¢\Ÿ(©á?ˆ¢ÆY?-?–,.<bä?‡¾Ç^Jy{AGN3FGL J1044.5-5737@qé2`o¬`?òx W À6·èɂ•qÀ:BÙ­…ߨ@z—ì¯@aP!«vf@~÷€—:¿ÞÀõ0̯¿äT]ã
%ô¿ç
€û¬Íî¿î‰ÿJÉPSRPSR?'y"z‡–¦?(ã*¤Øu?î>bMæ	?«VìλÌ?¬d–$£?«Kòô^4?5YWŽúÇ?TOtSÜC?êÜóÞ+q?·½9ã¤Ë>?āƒÛ
ϙ?·µI.ýVs?–vÁW—¤I?3˜®™"T?èìz±ÄU&?µdGŒJjv?É=zâŸ?´Җ0´?bÝóƒúYÑ?_æÆzM¦?í$/ë]º#?¥^3eRØ$?¶G'¾?¤ðÓ8é?'"LfC?.ö'=Õ?í`™el@p?·ÛE–79}?´ïj¯Só¦?·ÖÅ`Q6o?Rn;j	ï"?ièóö2Õ?ë]-:ár?¯ü¯(ýR?Âfn¡Úz?°Š|ÚÁä?¤ì»]AW?œZ'H+Xl?èá^ÿÃÃ?²ÞŸy'x?ÇwˆÖ0[?°ûŸ?l³iQ7ã?^KUbèð?ím÷3œ"?Öþ˜»'?³ª«ê:‹?AÊTìPSR3FGL J1045.1-5941@qù±_ˆü"¿äB% 3ÍÉÀ6´ýÓÕՊÀ9­Õ~L69@z§3
C{@4ü(+?ýÇ3½G¿Ò`x:Ï3Ú¿äÆëvÛÿp¿äˆ§¾öJu¿ç.†%HŽåOTHERBIN?l÷Rd­P?{|cÏB}ë?­p£¡ÈL?¶ÂÛ=2î?î¶þ{½Þ?·K±@j®i?M¾¢Ò"X7?_¨j³û41?Ý~tt?Á9˙­ ñ?áoÑ7ç‰?ÁP#'ð÷¾?¥Š˜ôÓÞ?™(|
&5?Æ­(he*b?²aüQ9 ?èüV‹¹?³Ž´T¯$ˆ?Ž¸ØnY?ˆ
SÀòN?ӒDxD?·ì,œªÀê?å¼ý	ß?¸›Fi‡2X?q=ñt™Qm?"á~ÔS?¿Dýq@›7?Ŏ̀Úc—?ëôän‡¥¯?Åî;çP ?^A'v®•Ò?q'ˆ&y?â.ª#á?º§²i§Â?ۅ¡'ÇŠ?» ì`³?®:¹Ex³…?¡Îù³ñż?ÍÎp:û~'?±Ê(^—/Ê?樸] Žã?³ˆHŠµ?‹ã|Ý8dQ?'á{%RY?ÛXóC%'?µ8q‰bÈU?áãøkÒÎ?¶øŠcóOMIXED3FGL J1045.7-2926@q	ÜÆø@9îσ³~À9:kÕ;0XÀ;"'»0?â"Åù/<•@œÈÿåí@¥bYât¿æ(Bn1y¿åÍa1É%οä+RÉGÿj¿ïÿÒ1ª`ÖAGNfsrq?ïùÎ9®U?Ew4T½?8QÙüéÝu?:[›Üò–?9=û–5š?;n"ì´©x?ï®õËÁˆ?†ÀKN¥Ý?p°Üãús?np$ðÇ?wԌaˆ=I?z *–MR"?îáJKŽÚà?ÌÇœþÒ?"Ðï×v›?"výœÕ6ž?®—mõp?'J/äø$X?ïÝ«tëíØ?p-AÏö/?G'¿±ÞÞ°?PÌWÈC?loÛöº&?mM'dâÔ?ïüõLÙޔ?1'a8?,®éO¼P£?)3!G G?#üL4ÿ%H?!ù;ž	¨?ïáÞ&Ѧ?eÖàÄ
Ô?Y™èêÔ»?Sõ¤"ž¨ª?aTŒ¨|+ç?^љ_i÷Z?ïIrØ9½f?€¹¨ªœï?‹PN)·<?vBÏžN?'Rû¼'´q?rŠc7J?ïøÐ@–H?M7À
˜?0–MîóMð?.˜‹	…{/?Dt·;\Ö?IÌyމ@RAGN3FGL J1046.9-2531@pèÙ'ÿ@=gqß@lØÀ:'8§ç:6À;ÉÙ³eº?ÌW'2_@cü3?ýŠ¿_&?궾ä½ëo¿â]'ÿ´'Ô¿Ä'ÿz㺿¿æJ£Ÿ#h²AGNbll?ïï)˜'©?[ñß{Z$H?CÀ«Lð^'?D¦£ñ6ª?WÍlþ-´n?VGZ•¡_/?î÷zVC"»?žÍ'o?'˜Ø17Ž?'mgä7?Žïº	<ÿ?"ØÅ΋$?ÿݽ­?Žÿ(zÙ¡-?ÜÒI%O?ƒ#!±˜K`?š:vámI®?…úCÿ­L?ìä鞿ž;?¨¯7){¾+?•T¼+%-ó?'Dÿ\˜¼?³ƒƒÿ9«?¥û½Ý
G?ïøLå¶Ó'?L1ÿnSº?2D»Á/ Í?At²iðˆ?Eªíú
?AAˆ0qª?ï"Ê<¤¡
?…¯é?³Äõ?{ÓwŠó?vœÁs՞-?zGÊKí"?€æXħ6S?ïY/ªMè?ƒÒ ·¿¤?'[—&Å?|äÉ`a4½?‡X~A/'m?vfðë>?îü?Ù+LV?Œ3@DÛ?Œ'ÅLÍN'?x W4Ú|2?'.¢-P•ü?†5|$6AGN3FGL J1047.6+7240@`׆@ €@DÀ¾ß¤?æÀ9ž.§³7ÐÀ;²Ä§d]x¿ôêeI/ôº@òfsÒ_´@mŽo¿ã~¢zòB0¿á币Õò¿à—í+ð|¿à*'ßB	AGNbll?ïý1Òh ±?-ÞQÉѪ?§RU†Ø?
†k#†?1‡˜åe‡0?)ÃW™Pô™?ï·\2äar?ƒ!ó¼‹?lâéЃ'?pŸO€6ÂB?uàqö	­Ž?|štvN¯É?j""`?tÝEM	›§?ub%Ë?a^•ƒ°?ƒ]3ŸX7?nqÿû¼*?ïÑØ$?qÍ´D:û?R
:?!˜`âÄ¿?wªªøŒz?pàíäÊ"?ïþÄZ|<*?Ê_XEKà?	åîùQ]?üÇãŒðy?è9.JØ?ÛÖËÕ¥`?ïåÿÍz³?f€Ñ#,+?V-®üÞµ?WOmEéœN?]ÓV¼?\j‰‡î?ïÃ3
ru?d1"×ʒš?iÄ
™?^™˕Þ?q"mŽÖùs?V§€ÈÌfè?ïøp>¬c ?F­Áa™Õ>õ
`Oõú>öE©LB.j?M–š>-þ?F"+Ú;OûAGN3FGL J1047.8-6216@r"ŸºEÀ9µ ÝDÀ8-r)HÀ: †ˆDÝ?öoôǽ™S@í/çú$Ê@<|z¿ãðÒ
¾¿èøò;‹
N¿èrz_'éå¿å3ø·P'¤AGNbcu?íqÎl	=–?°"½½÷X"?"%óœ©Ë>?š#zL…a?¯Po_rý?¬'6A=r?Ë»rGùœ?Ï|O.ó?Â=y•¼Ô?½Hd±þ¯?äß~*Rd?Ð0'Œ¡2?çۙ*«F¸?³ÇdôoÊ?·
u¶‡ÞS?£'®ePM?Å
àxü:?®²¿HLp?à²3f^Ùª?µV§O¼`+?¿Ò%.ì/F?³ß@º&Ï?Ö§ç‡@Ú?µRn«OÄ?ï©Wu:rJ?€Y-…¯!?i‡q"^Å?i‹¨9wtq?~Œ›×{ð?z'æwfX?Ù3{?ÓØ¿ŽºÈ?À¼:$Ð?µ‹¶ž`su?Þng$/ï?Ñ¥øøyÎÎ?ìéê×ú¨R?£‡Ž=m@?¤@¿!,?–à­´—?­Eþ–Y¯?œp¸ƒå^?ç
~]?§ðø{?¿ÊI˜X?¢æDqb݊?ÄJ¢}:_Å?¤9ÏÑf—MIXED3FGL J1048.2-5832@qöíÿ'+¿?⏣?Ïg¡À6Sà_PÈoÀ:ü¨\ªü@.¥5¯v@%¼`CÃ@¢ùš
WÈ¿Ô¸…Jµ¹¿á_6›L¿æs7ò#=¿ì8w{ó§"PSRPSR?)³'þ­_Á?%µ¢Ìø@&?ïHƳ->}?"A~+"1?–³ÃDŒ7?"-X:Å?%µ]+¯í›?=º|S¶?ëw-±>&?²
ÔåuL?ÂÛä}ÿ›?²
bàR™?zM'&Ø	Ø?s¢Ï	ªY?í–W<IT?£H'ò¹Î÷?µ¾t%ˆÿ?¢'•<ˆ^˜?V.ûîód?R
çú£ë?í{0f…p?¡@s¿h«Ó?³Í¿£qô4?¡¯3|Ë?ö<#ýÖý?!ë¹eù¼?ï"íîªà?‹²²6¢?Šˆ˜øêï?Œû=cèў?K0¨Åµvå?cGÙñîc?듎¥þ4?««¤9 r?Á–"¿Èµï?«©úªt•ü?€¢
__ ?ƒÚæíì¡c?í%ÎÐÕgr?£'ºæÇÿñ?´½H/b¦æ?¢Ÿ\jþÀT?^ßhšné?RSÊ\ûó?í£†Ê¬Y?—÷Ÿ·ªv˜?²hv'wÞÌ?—Ï¦¯PSR3FGL J1048.4+7144@`íßý`é@E#,?ùëÀ8ªE¹GµÀ;jä'Ë÷»?ð"……æ^n@hðÎ3Õ@"m`*¸¿âp4؜0D¿å·oK
¿è'µ"9¿æ€¾;x.AGNFSRQ?ïó¯hâ?Tuq…Ï?Qe¼"ª­?Q‰Ü3.m?>yçs³0?8æº>X-j?ï;Ϗ[
?˜'²'¯Ù?†Žmw™íç?'ßþd÷?Š©ž²M¾¦?"{•<?îì(pB¶?'¿ïÿÛ·?qS^ÚC?ˆ	¼ä™¿|?'	žñ9—?†?Æ7´¶?í9a釡'?©wÉ×AH?¥ŒU\'?žÌéP†Ã8?¦ÝŒ	Nv?£ø¯Ìnè?ïûƒÞ¾´(?:Hê6˜"?8ÿ‡
ï`O?5-æ¼´a?%ÃF&øz?"¯jS–X?ï¯Ú&ÄŠ?†GÞñ$‹t?vίO?l¢Þnb?qýµµ÷y?tNëÐ÷À?ïi]ñ;°Ê?"DÄ-«"µ?"êêD+þá?ßpV²?€½™jØ
£?t#-dcÃ#?ïa‰Òý?‹‹eŸ"7?"	-u¸ú—?u*pœÃ@A?ƒ"]Ì
Ct?†¨×—ÂAGN3FGL J1048.6+2338@j¦ôÿ†]}@O/ »èÀ9¹i,êCÖÀ;½WQ­D?ív½µhé4@?mÚÎî@Nvÿ»·|¿¥Ÿj7_¿çÏà0½ô(¿â͉:¦Äû¿íY¡ÃAGNbll?ìlÏ´]À%?´˜~…?¹±x)ÿ¥4?³Ý!"!FÓ?‡@Q•#1@?'GGÏØ3?ç^ŠNøá?ÆHŠˆY«B?Ëv–à,?ÂÑF	µÇ‰?°üü¿ž?­žÈSQœç?薼½é«?²ÕŸðèäD?Äû©À>…2?°-¿§â?±RƎì­Ã?ž:<úD?ãaÀž*D?¶ËSѹ?ÓPßìöI?µ_W È.?·±¯ù5;?­°ò}jÍ?íüuöX?§Í³JÇX×?­#¯nf?§˜(«Dè?x¨€5à?tՆ"ù?ìcÔùõ'?³v/'Ĺ?µbör_.i?°ÆRÔQ?ù†ö(9?—Rþ涔?ë¹=à|?§éB?ººã5‰?£Ü)m(û¶? T¹Îiñ;?ŽëéQûÔ?겪GøÎD?¢4£ö"ÇM?ÂB£ØQ?ŸX(jj?˜²Œê§?)éŽAGN3FGL J1049.8+1425@lÝ¿˜0ä@MË@ÒÎÀ9÷¿µ'À;˺µsô?Õ>vn3@Ëãæ™Òz@¨‰?"O[¿èÈ蘟¿ã€ßxöáÉ¿ã<æü+'³¿ïÿÏ7؀×AGNbcu?ïõ	UOxõ?QkqQt¼h?AǧQ p?A[JÑ;^!?J˜
Ú~?Iߕ—›¦©?ï&!@±9ã?"z³~x—?ŽY5%¤ö?Œ=6›Ÿ?ˆ."=S?‡Ô=è'8?îC@=vœÙ?˜ñ}q†Ô?¢üÛ?"ëýLÙk?'uþ¡ë~'?"ñ"øè+?ît´¢´uh?˜à#ü"?™‡ûÖ]k×?B^j¼´?—áoϤK,?w»†%þ?ïûä/…?6ÂGJIB4?1™¿ÁŽ<?,ϲ­¿|?.‰ƒ€ñÀ?*öéœ_sb?ï»5Gé?uGØ],•?r{³óÁ'?hiô6{q?p*éÄDŠ?kÜ-˜_¡í?ïMÌDD?‡™§T™êŠ?"p`…éÈã?'øÛ[¶­?'×ë{›ý+?qï!þ?ï¡N+(š?sF™eðá[?}ú?æc»€?h~z.%±?q^ªŠÎ"¿?kRÑ¡¦aAGN3FGL J1051.4+3941@fMp€0<@OjÀh:|À:s0V	!À;¸Ir9Ù@?Þxš¼ü˜@
—ÉøÜö?ú¡I …[Ÿ¿ïÿëü¨:?ïýøÞp¿ܮ'@òʟ¿x¶0d]ÿAGNbll?ïà†8¤ó?gÍÃbÚ܀?RÝèHÁIh?N»Ûr[?f…«9wð?bOlYFM?祝9Vkz?…÷ٙM"??s«~«Ò
_?wÔã/Yq?w‹ä'šà¬?€`à"y¥?îöx{M?†Ã,¹<9Q?ˆ×ÂÈ\½«?z0"Å"ù??"Å2/ϒ?[ÏXhÝ?ï7EÍ¥Ì?–
Fså|‡?'	­Ø߸^?'< ;eh?‰ÒÞF¸D?‰s ª'¸?ïöïðŠ¹y?IïV¨ÁÀ?5xq""ßJ?1=OAô`.?I"ñˆ¶á?D•}Çñª?ïá¹ë–?h¼ƒ×xô?\"°·ó?_	¢Ü,?`7IØ8(L?^`82Ͻ?ïs¤ Ÿ÷p?~ëçù²¶²?|µîH!sÄ?tÅ® ?"¼­Â?v˜$ŒlÙt?ïÅ^À™|'?qŒÙ«L0p?râU=}È°?kI…ãäÖV?dܕ¢t<?a0køâ'~AGN3FGL J1051.5-6517@r-'Ÿì™òÀÐ3³À8ҙ!¤•vÀ:ñÅÒ݈¿¨~".xðI@û)/y?@Äb¦-¿åÜ©ì£ö¿ëú¬{ôm%¿âúðcLM¿àš_ð´AGNbcu?ê1¦)06:?ÃaØsZPë?qŧB
f|?km½?«-?Æ«: 7X?ÃZ1ÂÎNá?éGßܧ"?ÆîLA?¢ìSx=¢z?¥±)ë~?Æ(ã¡ÙÓ?Õ!"?åÙÃz`Ø?·Ooiÿ??¬0yÇüŠS?•sϛä@•?ÐÆiҒŦ?¶Z4"x?ç|/%‡y?±œx¬ï?'äÀg_ ?zk[¨Ó4y?ÑKá¡+o?°Ôa©ƒÀ–?ì£ÑC¡b?À$ŽÓu'?]ÛR]Ý6@?U@
¿q#•?ºo¤,‹Y?À1Ë¡uþ?íÞ@lyn?°ÁQ"Ýù?Œ["²˜b?'fZ¹Nœ?«|®Ï?«·Ä"G?쫼é̙?¥Ö¼ˆ?š*H¾?ˆ®ñ€ÇvÞ?´Î$Ä81?¢Ó¤ÈÖ?ì¦Cê?Å?™<ZQľ—?wæ<îÉzö?c'òá׆?¹O|ß·{¦?˜¾Ë¿l`AGN3FGL J1051.8+0105@oD  ô×®@I¢¹¿©Î›À:(48ñÀ;¾º•"<¿ôÉ&úë™@¾g'‰«@…n€;N¶?à<LCûWz¿èuzýŽP¿Ñ蛡¿ãÙÝu«A§AGNbll?ï󭽤!?V¡:Ôè|7?2ܙj³?5G}*÷yú?Sí^³®´"?SÛÁ¸8¦?ï˜dϧ6?Žœ-In›Û?xA'/¡Z½?ƒÊ&ì1MÌ?{Œpø£ÝÆ?"lõŠ§×?îä÷Ìæß?ˆyA"?†cP¢ÓÖ·?uTKk—2v?˜M˜¶±½?ƒ[IþX?îã'Ï[P?mÆÉL?\äÐfĶý?_>x'½õò?¦ú¡NWI?œ÷ÆÔøM?ïúªMyÍ?@õŽz®—¨?%'=€Ü%J?&FkZÕ+F??ìv¡~ëw?=·U	qŽö?ï߁ÆFÔX?lp'ñ8Ïn?\ǝ+Ç?X°Ð…Ož?bX©ãá`?ffª
 }?ïrëÔò,¥?xxÂå/'?zÉï~þº½?g8[!
ð?…àõ‡o?s~
tLK?ï³Óõæ:?u8€Ž«Šû?>ˆÈ	")/?6€d·?'ÖN2jo?tã™{b˜AGN3FGL J1052.8-3741@qf[@-¹@3uÑÀQ"GÀ:Aµˆ©\À;¼óË>WT¿ûrßsB—Õ@ˆnÙ§{¯?ÿðŠß—¹¿êք4ò>æ¿áž0I@]5¿Ò0¡Ðl6¿Õ-îƒ^wAGNbcu?ïû9{ï*?6üo"?'ÈÁg­,ã?t§êÍGé?:O¿[)?1¼1hy=ü?ï¢Ï¾¢EB?ËP¥ÿ?m@ö¡þ´#?m
óc/"^?÷¥d½<·?Œ™:ÀSŠ?ïž-ێ?"Xÿ=<í`?'ú3«?nd¼äš?"Ã=;{ªf?€pMǓdè?ï™{#\£?zs4%´d?emO{!K?s]ž[´æ?‰xlehkx?z^å8Š}J?ïü±ð>·?+.ꎀ?yé}>¬?C
=Îâ¨?2Ò8¤àåv?&[b¹QÝX?ïÞ<0‡Ý/?k"œS'?XÎ 7­¤?UMNöé?e\¿8܊Æ?e€}?N%#?û€G?oHw;ˆ?w
âÎ?_{øa	·?'ÖüÎ'?gâ瓄?ïí-ì]œú?Q ÏÒguÃ>ü7¯Ön"­>õšÙmFg?b™¤2M$ä?QZ­¬"JAGN3FGL J1053.7+4929@d*à~Zy@MŸä6vÀ9­µ|N/8À;'
ãˆÐôÀ .s±@mwô-cæ?ü»È€aå"¿èˆÂ¬bt¿Ð¹9#¯¿Õ,¯Æ¯¿á}"ð+2AGNbll?ïó@kìz?\]m¶=FŽ?3«ˆ£€?5Ó@*9?T"GGÙ²µ?ZO%1³Æ\?ïÄÃ-ç™Ø?€N‹òÈ¥?iœ$"µÚ?qá¦ÿUܑ?pÐV´Š"D?uh(·ÉûJ?îÙ^è1›ó?'úâö	%%?ƒAš\¼Ü?€(}h.¿:?›3UÆDÃ5?å÷dæ?ïÌëvc½?t3
6\ýï?1þÀ‰?"í·½-MR?y5|Õ»Î@?t"ºÃP?ïûV:&ö?E¨=)ry?&›€	1ÐZ?"äNÖ·?;·j$ S?D!³¶Hò?ïéçfùU¹?bEÏ©"2?SlPǍ?QŸl¤ƒÏ?XÅ0T;U"?Wâã®Ø?ïeAÐQ^?‡\ü#_R6?z»ËK""?zñmF]0?‰Q¦L¾i?ƒN³!&?ïôŠ½Ñ?Q¯6np[>èk‡.^fð>ôK?ºûÿË?V¹®ÇZs?Q£…dlAGN3FGL J1054.5+2210@k!«`kz¢@O‡@`B_÷À8ÕE!r@À;'°Ql^¿òž"•P‰°@¸'uåµQ@šþ¢Lœ¿äÒÒË?¿ä M¼¿âJˆÝ½=–¿à]Åsù2BAGNbll?ïúĀ´,?A¬ŸwA×á?sÄlp?"?9]òž?D²‹Aqˆï?@Ã]Ìýr?ï·U+Ör"?‡(Xª4H;?p…7¿	m?úÁ{¯©ž?t7äã6ù?vî.ÐÜ©Ÿ?ï<Ïx<–x?†Ññœ1pÞ?€  
3¬?qÃÍè÷?VñE?ƒkʘÝäz?ïƒ@©_×£?"˧¿¿Kš?D D?ëO?IóàzÎÁÃ?íÑs2y:?"sÜÇôÒL?ïýçűr?1A¶ PÈ?Ea—­¡¶?¾a<¢j?'ëöâ+ó3?-~Y³?ïæÖø?iÝÙT¤+?VaîÙ¸?WW#œJ ?[Ä®
ãào?bD¬ÀÝg9?﫤ÞòX?r´¦ó\?pè*QßZ?]A¶"+j?y«¨hS o?p	µy1¹È?ïèßÐ4¶@?bb¢ïÔÖ?¤½ê?ž©jcL?f`Û<?b?Õ2¸AGN3FGL J1055.8-6025@r*@ºˆ¿æ°ÿðCRÀ8>öJt˜XÀ:0ÞÿÕ7Õ?ÿ¸VÉ}÷@μlØE|?ø¥ˆX‹¿êYÆO°‰¿Ç;šNº"¿å8BhҞÀ¿íú±°=PSRPSR?9¯j»†•?8rW])C«?¥(?²¨¹E/¡?¦³ÚlZ?² ݼ=›?gK'ù
.Ô?d£oe¦i?ߗšÀŽ·?ÄéÔ/Ãç?àçhÍ~?ÄîŒ_ßA?¦¿c–=Ê?˜÷J¾ƒøŒ?å{³ÒL_÷?µ`|´Fô$?Ò0µŽ†"Ù?´WVŠó…ì?¦ÌŠ_P.? Ü.;=?á}ÚëëÃT?Ât`'?Ú*ɶ܏Q?Ãòh4>?&åÙ°Œ4?+guy˜i?î1J>"á"?¸™?'nj'?¬ÔwççÖ?¸–9,¬?wæ¿9ؾ?Ž*²ë6?â¡w1?¾y")´ž?Û`ßÀç³¥?¾µí¸)Ҍ?²1³1i[C?¡˜‡?åcµs-¸å?²nÛÍ=,~?Ь(M¸*å?°éJ?•÷a?§‡aAe/?¡©@@¶?äÁ>GI¦Î?¸›2BiÔ?ӌ¢…{}?¸¢l©óð,MIXED3FGL J1057.3-2341@pý8€®@@…ߨq¤À9ܕyyh¢À;·ûêlj—?ôgë†Ì7|@Âó5AU`@ˆàdõ"¿Í¹fb#zr¿ÙŸ
¦¿í~×?'ÄP¿Þ;Ê®d'AGNfsrq?êô9kí ?ÃZbOËÎ?Â#êô]½ÿ?Ã
îiˆ7?Yzß^
Á?šãóă3C?î²ôv+wÊ?®³}žÐàå?•6!$<ö+?¡»qן?"kP,¦'?¤®¼.ƒ›â?éî£C2üú?°†d%_G?ÀTÄü&Š6?¬ÀäÔXñÚ?¯Â·Ýî‰?œÆ‡,á?éC¿Ý/ñ?½T©©ËÚ£?ÃI\C¼‡?½—bиGb?®ž–îïaw?¦eáÐýÏr?îzÍT­?³7ˆ'
Ä?¥±%]yÜ$?²"üî?uknc
z?'Tµ?ïŽÝ9<ÈÄ?–4i.ν?}Ž6"õë?""ìê 0?{EF"‡¼?‰Ðh(V
?íA³ÔƒP?¢,è6!߀?¯
¦™~¹?œ]gÙù?Ÿ¢|O‡õ?'R/àˆån?î
xwyÎ?¡›lÀc+?¨«½*êО?©êKX†?‰ìí6vJ?ˆ3ô®¡AGN3FGL J1057.6-2754@q$±Ào@<{Ÿ³À:w•¤A"HÀ;ÌPwؕ¿ãÍç˜ÄÌ@{f°6?þ,TßÖ>æ?èvK6gΤ¿ã%ZºÇοß@‡ë­sҿ̎)‡ý~µAGNbll?ïó!ë멏?QîIöyñ?0Üü³c±?0¤¨Ì0ZD?U"éWs¹ž?OJ«h>`}?ï©4@"2?"Pµcrk?qR§*ˆ?mgÏëb֎?zz1­?}Qx?ï8Ã]•æ?'6›º´…ÿ?…"œ›ýX"?w‰!b4'[?ŒtrÊ`?u†¢Î!Ì?ïQRìÈ&?ŒÃ\È|?FÄz úä4?LLéuS`Ñ?•~@éï?Œ_Gµ·Œ"?ïûm	ÔÑ9?4h$òÂé¹?!¬Ô¶bF?§À0‹…±?<[J]p‰?1dßL¶?ïßÿº4ï¡?j6Ö<°0?Zo7ãt™?S2¤…lyC?bñj7ì?eÖfß-?ï™T°—ž?o)nӒ?wžÙà^¸?búu¨~Þà?{ä6âqz?c}P¡þ?ïä7òÍy?a*'ÌàÌ?*¨9¬LÔ§?";*
?jl4Û Ç?`ÇË«™‡4AGN3FGL J1057.9-5227@qßÔ§e4@"àà*!½À5öU/}ÉÀ:—«bï¹a@JÝð
¿w@nFM—7•?ü,y¦Žu¿¸Ú§MXŶ¿ÜáåÂUê1¿éL)õØðÙ¿ï¥Ó–7óPSRPSR?C$üÊ×É?Xˆå×h
?ïb8âÓ'?˜ˆ,Ð;ÃÛ?Šµ!ø\Ïb?—À—Oáku?;£8}l·?d·5•Éål?íþÀS±qÁ?²uðD'£ƒ?¯ÝÏ^ÎÐ?²nÇG4™{?Šýø"YÃ?Šó'Ä.'?ëº"¥ÂO?¨ø.žz´9?¾ÐOE¤?§'µ|Õè>â})\°Ð±?7dØDË?ïñêfnQ ?aø€–¨¢?\9FôäJ?`ï\—ü"µ? ðk±oÈ?*È_"äÚ°?'¨v½?šlL̏ϼ?‹'ôn9_?š_•q?R}>iO(w?háA#Ø?íÚc'u)'?¨ëƒ7«³?°âîò…{Ò?¨w溋a?˜›™ªA¨?"x¬Ìí¨?묡]ª¢x?¦ïc7£Sƒ?¼tÒx)Õ?¥`~4>êÔÚߤ¨h>ëb¨¿'Jº?ïíÒ°*n'?Y¦æë#R?b{-vôg?Y†&júPSR3FGL J1058.1+7010@`ûrà\̊@EÿüŸù/+À9vëg†ùÀ;à±û.·¿ã§|p¾Ùð@Cٗá]¨@ŸÜ TsË¿æçˆûÅ;g¿éO>	X¢¿êùNñˆKœ¿äÆMy'AGNfsrq?ïùÂ#Ús?Cô'9õ{Ò?;vÇ ?;pQKu?6x]SW?5%ê2›¯?w_Ýá?û÷Ú-Ç?vፋ²½å?|Ø8iì–`?~Q¶ÇÍíˆ?"´VìóI=?ï,3¿¹Ù?…NÓ~•ýÆ?"Ðt4æQ?€LIÙ—?ßtØ	»?y¿XN¯hH?ïP]æe$G?ž>‡Ï0?qS8O|\?qÖ7èû/Ï?'Ÿu%Æä?ŒÇ÷4†BÅ?ïû5íïÿy?Fº†Ÿ;Ê?6»ÿ7<´??/C¿n.?/)%MA?5ß
aø›½?ïÜ!ô6?qøÛH"?^³$'x?a$Bel?d"'£¹N/?hª"ξ¾f?ï™÷çœu±?y­á_`ú ?xWXÒåÁ?vlƒ×ՅS?z¬³SáGé?ee.ÑLTí?ïçY´ê?f½Jê…'›?<V8cD{Y?65·#¬4ê?eU߶®…>?eæwñc½AGN3FGL J1058.4+8112@_ÿ+@öjU@AdË@ÒÎÀ9…Aî·Ù À;u¾¹å?Ù!Ââ,[@NiÔÚã;@T3‰M¿éò«ð"7¿æW˝;©h¿ëx`!ÿêYþQæ7éAGNfsrq?ïü…'`†?7ß±Ãâ<?8à\Í9œí?5PÃ{IÆÞ?MårèëÑ?$¼NËÉ?ï¨cG*¿?ˆÚ,ï'Ó?s›G·Ð˜?'H–ÿVÓô?xZFb»«?{š·º` i?ïë&ݗÿ?‰9ÖTNЌ?Ôý'Éh*?"Ð,oøõð?Šp8³`ü*?yàå<î
ˆ?ïXÔi=4?Š?v¸n?pâ?¾'?iôÊL~ۖ?ÄúL` "?ˆVD~`ãX?ïüyÈÃÓª?5£v«?7Í9ꔁ?45WWW8?{´Ã¡îè?Û³pü‰?ï߈<é¯ ?jp½¢£[¢?\
"Páf±?U–¥ß¨:ª?br±äAE3?dñrv§•?ïbŠ.A²?…"œ±[j%?…Ð	9±ôÒ?¨Âú=?">…0µ?{r­•¦¥.?ïÞ§°ˆžu?cqñe,²j?RáK_¨õÁ?DWìÆè?gç©£Ñ ²?`؉éØ1>AGN3FGL J1058.5+0133@opŒ€A@Jc*`%څÀ7s\#íEÀ:µ#I±#ú?òè³ÍøE÷@Ð>â¾ÑŒ@碥0üw¿àã ïá¿äoÒBW"¿ã•ýmt¿ââ0-¼ž#AGNBLL?ïûV§EmŒ?@DëQP4`?*!.ϯ0´?12eâ:;?8:/Fpz?6ҘΫA'?ïęÃ=µv?u››ýü?i
¯­b'\?ng&¼¤i?q,F3«è?v4}OQòõ?îêß´}m?•4L	"=[?Ÿ0³nZ?‹!à¢#?"Ô‰[hC|?F,Ëj@?ï"s祸ƒ?'jÙùÂ4?GP,Ðí	?RΧ#&X?‰n^q^ï?'NÑôç'?ï÷~G_ã?xÿ4(9?BF¸"…?lƒwÏ0ˆ–??ۘò¬?e݆éË®'?ï譝;?c%Û1@¡$?Up lí¢.?Sá†@??Y59ð'?XLW^<?ïD>«·Si?ŒïC¿ÿQ2?‡ãuR3öÊ?†z—ì]p?‡ßÊFð?'°år®pÞ?ïç W…ÅI?bßxlæ~??gã*ü!p?>@xÆÃ??dò«î'Ây?aú÷¥nAGN3FGL J1058.5-8003@rŸìºËCÀ2G?}ÄQÀ8%ðT'RÀ;*sMÕué?öfnSŤå@Õ	2®¨õ@óaDéi¿ÝÛ³'×hæ¿å¦,áÉ¿ä‰][û©Y¿çØH»/ÛAGNbll?ïïoOªHz?VXV×rÛ#?CZ2@3?=YtÇùô?WtGQ¯"h?R©²$W³¨?ï*a`ÿ/‡?š*Êâo~ò?{-‰â×¥?ƒýBŸX"Ÿ?"ðHyÑE?•'£&îÓÉ?îÔ¤<_׬?@0$h¬?=ÙÜ(*.?ƒ³ê›D_›?•-žý¨]?…6*¼õœØ?îÙíÔ{º-?™ ×{|x!?t
퀂æŠ?ş]†~Ä?Ÿ¾Ê4#¿?™‡«W¢?ïøñ'S?H3ºTOI?:óaˆGæ?<ˆëw$mš?@Qëžh¤ü?:B´³úí?ïµ8_S2é?IµÒè?eF:'s›?`kì—7ÿ?zÀƬͶ?}YÏJD¹?ï[¿‰B^t?%Î¿3c?"¨‡=äv"?t/îkJÈ?"g–jüª`?sf60¹¿S?ï¬J6ì"?|<'l(¼?i…X)™ÏÈ?^#Ë/Â|?}8XP–ù?yÏî¤UŽAGN3FGL J1058.6+5627@b³fàé´@K8€iFëÀ7é´[¼¿9À;2¥n¹òÀ  :G¤"@'6MïÍ?ÿ€y¿ß)²_§õ¿à½0o‰z¾¿à;QÈÕ¿¿×'m½@AGNBLL?ïüª¸]ü?;1uÑÅ?
#\0(í#?@•ÉE¬Ð?7Ô;£Ð'?:mñ^uUë?ï¿ »ç¢?† 8"Ã?n,±-›Ùå?ÅLÇ=?q§uÚ?s½¦2ëúä?ï]ó"WÏ0?Š¢ROÙ?x¬Æ†C?yZä•$ñ¥?Œ,»¡‹"b?†1;°\'?ïᘧ<?o'¡cÛ>ê…ä@ý?	h!^?náHùNÑ?o!E­°¾)?ïý¨<I²Q?DmZÈäºô?^¿sER¯?[™£
)?/d‰À.Ý?DWÀo	$?ïèì''ƒŸ?fÄv¼EÓ5?SÐÙæ׋%?QôÇ
=¸?ZV×})÷J?a)etd?ïv1³^ð.?ˆTY¡æ?zHÕÆ]·?€=À·4?…O(ˆ/?'£õ/ç)?ïø¬9.tÝ?RëœQ¦>´QG
ÂïD>Õìt#–,Ø?MDó"á\'?RêÏléP$AGN3FGL J1059.2-1133@pšÑVŸ@EYá @è(À8AëÒK'À;4]"<?Þr!+û1@ÓrDëíN@qÀa¯r¿Þ¶šm¡e¿ã/ØñÚ^—¿Þ"]
]qÜ¿æîBøFAGNbll?ïý/<•?(àny·$e?Ÿ°Ê ?[HMŒá#?.
îÆ×?$,#+e?ݯ?ŠYÅ[?vôŽ<+Dö?to8‹Ñs¿?€Ø7W»ÃÝ?…ÁÞa¯Ý?ïS^ëY#?†Lt#¦à?{ÈÝ{/?qlK'Ea?CÖeõÈ?ƒ'¯¡[˜w?îÑ&Q¬Ï?–›Ps¢ô?uM0dí¯Œ?si¦uÕ? CñÚ=ò¬?•¹ÈxwF?ïþ±/|3F?öW€Cõ+?J¡,aàK?+jW#Ko?qr†BÅ?­KßCË?ïÖ×Ñsáµ?p"ÔC?c0n‡È
ñ?^¼ÎToč?e÷À#ò§–?håËÛ
î?ï¦ë°×gŸ?w'»H$åÈ?qvÚN€ñ¡?jêp¤Ö?{MS‰®¯?r_'y1íR?ï­oâ'J?w13X6î?dy•Ö^ "?ZOKU]'k?CÆ~á?vY¸äP¸AGN3FGL J1059.9+2056@k'_ôö@Oî2à'¤À:kUž˜À;µÕЁ3?ê—×p¥ëž@gßbP­@Œh€Z¿éÌ,QÓÃr¿åÈãï(Ah¿î±}cX?é€4
AGNfsrq?ïègýŒª•?o7":ºß
?aïDəÁ?g؜Wͪ?F¢÷6úlò?T¥&UUM?ï¹l\…Î?'·
Sý?n̆›?qˆûÿ¤Â@?ts㍿¬å?xº{îæ5ª?î3ਙ3?–æÝr¡%?ž1ô–"?üÉ©Q©ˆ?›†QúYß?‹ž|'\'&?吏òkdI?×([Ãê?aódê"°?ˆÜ¹Ó©?›j8´Ð¢?†`Pì\?ïí¼Çy¯L?m¶'Çl?Y­Á=¨O;?fxHòa?E±`\¶Ø?TϤ/W+?ïã6š.º?p.‹

?ZÝg«áñ?ȃIY1j?^µcАû?cí!WÈѱ?ï2XËPÔ?‹²åhğ?ŽŸÛ(ådd?…&K¨¦Ñ?ŠSŽ¤Ff"?}%§Ø?ïôÄßmŽ?plBŽ°?AT4aeÞr?dvûþtTÞ?Nx¸VÄ.r?cíӖä2BAGN3FGL J1100.5+4020@eù«ÀãŠ~@OÌÚ`3F~À:
µÙk@ÁÀ;¹u.€F¿ê_hè™(@µù÷}?ý]À?u¶»?ïI¡¦¥¾
¿çÐ2ÈTB"¿áZœr€À?ÇàE²^.AGNbll?ï÷À[O\	?KÊ<ÿãuô?%WùY?#:ÊM§PF?K¸óoi"?I¢U='/?ïÀc3šÐë?‡²Âµq¼[?mù‰9×?ƒ((5þ½~?pÑÜÛ}‰­?së=';
>?îþXžZQ8?Œî¯iè?†²cËôŽ?~üfkZž?"ÛºGÜZ?‡"˜'˜—?ﴁÀ›!j?ƒ'¨¬~?qÆ,þÈi?.÷ÃıŒ?'¦¬][ÇÇ?ƒnrŽԗ?ïý?†Ü0K?,ï_-WU†?C,d­	ù?åÅL8rQ?.eÿìš1t?'g%j??ïèy
ØÌ
?f[0‡š.8?TXìéçð?S*-'ÉR?Z´ýü"EV?`v˜'O—?ï{R4ïæ?€–ˆz‡åx?|Vf+< ™?uö	"
Ôþ?ƒ
¸fĞ@?x̎çvŠ¹?ïö"榊?U¥k»a(Þ>øؑŽ[R>þ»-ÒÛO°?R•»BZ'?U‰	¥WNAGN3FGL J1101.5+4106@eÁŠŸb0@O½ÿôA†À:U€[À;Ð>åE¿ø¾"y@JDâˆõ?üK_¯+¿ésã@pw¿ÀƬ†J N¿Ûï kfg¿»|,êLmAGNbll?ïý˜Ê;Íá?$ûâ>àg,?Žµ§j?.QB{	?(,ʊÀ?*Zƒ9Â"?ï¿0n ³Ä?<eðúpu?j5gÙ)€?r©Íåï½!?sM-uñT?w¶¥ø†fÇ?ïu㐢hå?v'ÆLG?{hCÆi¼?hôùõK‡?"ÒùécÑú?ná¨GxŒÉ?ïçj›ª?bÒù66ó?…²"TMe?pè"ô?hœ2~B&?b´'Ðc?ïþ§Y'-?>2£sª?'8%bU^?bÕÄlÆË?'	Æ3?qî'¡?ïçu.1Ä?eUg»ö?VyT˜¯?UÛ}c0é?ZœO¹t(
?[ܱ‰Ïö?ï±#ÝfY?h«Ô¥£Y?q'ºÍ"âs?Y³If!b?uÜV'˜¡!?c®
‹+1O?ïûø‡C^W?3áŽk"}â>äÖ-–åt>ß~w`¯GQ??•HûÅ»?3¶Tî@žzAGN3FGL J1101.9-6053@r ¿p¿é±}À9rÀ7Õ8[' NÀ9Ò%çñ?ý'¤ö!d@	1‡úŠË @	¢®@D¿?â̤žZs"¿àW6³t ¿è…ÂÖ[¿íUç}¨!rOTHERspp?"WVËÉÀ+?!¾"‹Nc?ïëÒv"í?¤‡ë8¡è?=ÖüÛÆ*?¤É3ß,U?%T[ð´?W5ÇN–»?êoMª¥'?¹Oä0ûý?Æ=t?B
<?¸ücà@õ?‡èË)5bË?|w	×Y@?èâ±!Ü°?³©'Dœ£K?Êù‡dbÖ?³Osl?T*¤ñGõ?VS· ‹æQ?çXÙ8H¤g?ÀZÓp]"?Ñ:"êÕe<?ÀZ¸p§æl?Z°7Ôo‰?ÝJs«v?îY5­y?·Jî%ÚB?ªh'[T	?·IÌdJ–ø?#¢˜Â¹ƒ©?BóYdæ2{?éɗDw?´Íx¡`ê?ÈÔºJà?´Ð¡aœÏš?f'úü²"?Š0ùöeG?è͏Ը˜Q?±(*‡?ÊÓW~Iº'?°¨¹®ÆÙ?[qF'yWŒ?]š&L9þJ?äƒMޖ_?¹ÇÑ
U6?ÖÝòüƒÁ
?¹BtÉÊq¥PSR3FGL J1103.1+1155@mÐ~KZ@N4_²?À9œ''%àÀ;Àæ"ß(¿÷ÒL%r€P@Eõa™š@#²`dä	vW0y¬¿çàVqH9!¿éFûzgص¿Üê¦+ù-(AGNfsrq?ïþ1sü?$	½Œ°<,?èv5¥?èW'‡£?$Xªá.,?cQŸéô?ïÄP/Bc?~"ã<mt?jY|Œ-Kn?nåzù/~5?pË'Ê÷?t£W¬ø¼?ïQ*g\°…?|Á–ö?¤"?}–w™ã™?jž£!`U‰?Œê*¡V`ç?vMOËc¥ö?ïùsK"Á?K_˜ŠQՑ>áA`Ɔí>ñˆãÈY'?IE-šŽª\?KJïðI?ïþÎ	7â?dG="'?5[Ÿþ\—?TÿáÑ?	yfå?câŸ		ü?ïꊵ¦§?dpÆøª­?SPÎ-J¢?ScYEàl¹?W™Æ$9Å?Z¿Fwî¯?ï®3ôÈ?dØAQp?q)¿°qYÚ?V¢¨Á<¼?w¼±Û´Ž?[I©˜å?ïÿ–‡žù?%ˆÄ²ã	>²$È ûú*>À)‰Œ1
?"•¨¢Þû?%{‰{É0AGN3FGL J1103.5-2329@q×®6	@@‰¿¿ž!À9á¢çrÀ;lelkc%¿ì¼A/±Y»@Èvç'÷?úPúa¤¶?ïõz?ƒš÷¿ãx39W(u¿Ø;âŒÛ"Ù¿¶y‰âJAGNbll?ïÁ\FÃÅ?{Ñ'®ÿ_,?P"N£Q'ô?Pº ¢éη?{I^>õ_?zàZQ3?ï¬ÆäoD ?‡[QuÁ?o!W;ñµÊ?l—Ò·£?zâ(U?ƒbHtñp?îAWJŒ¶?"du>~<‡?'äÿù"âó?}眑ݗ?¢xX½u0?&Ðå\?îqL•Ò1? I¼Œ?E_"œ!Ó?PÈwîC(?­ãlæ! {? ;•©»t?ïèö]·7²?iµY߉ƒÈ?Eç¥ý3?IЗ	ÈJ\?aŨ°SÀ€?e0[)«ÑÔ?ïàó)Æõ?gG-¬"¯‡?ZèÙNa¡?RýȳY©€?bbZ\?bËÝØȌ?ï>þn
,l?ƒ¹ðd-_?'ß@aØÙ¿?s^-Õ̵Ü?a$•P?~pùö§?ã?ï'Z/mÎ1?}>©7×?(¥ytï?!‡× Fô?‹FÞAÜqÅ?|ð}ôÕAGN3FGL J1103.9-5357@qöÌÈó#@—Þ_ò.À7ø_ð*ŸçÀ:׀·J"‰?óˆg¢Ñ{³@Ö[uòu@$6ým(¢¿àOéÜÊh;¿âý#6pY¿ã£¨™ÅA¿äfÈ\¶ËjAGNbll?ïÐ$›îÐ?qâïéÿWú?=?ð;›^Ê?7yõ^™Aö?v³t|ú¶?q(™û²?íӈH–û7?²	ÍòÝDÏ?…Gö‰–?ˆ'Ø·çm?­‡8a#+?°~À².³>?퍽³? !lF±1"?–@'"Ë£¤?ˆcÞ<‹Ì?¬n™á?›]¿9@‡g?ìí3~e>?¢Ð@R^$V?†§lû\Öe?Z˜Ë;Ú?µÂàÂémC?¢kuX—|Ñ?ïó£HD}?R«Lƒî	ÿ?-0?Í)ã?&'HohÌ?U)
Á¼Õ?Pɗ¹|?ï1µ¥qq»?¢c˜©A»?tš‹ÉW»h?x$™ØMÈ?"¢¨a¬È? ¦RÏ*¬?î珞ñÆ#?'˜ Viq?‰Å¤zÎFW?€uPP6I?•(šË?Po?Šzãͤ ú?îïõAÍk?"u(r§H?7Ä ÚÛ?mÚ5œ>A‰?™eu"ú@Ç?'Ëð&5AGN3FGL J1104.3+0730@nµ‹¿PãG@Lõµ ÝDÀ9'UM9oÀ;­`˜ÇÃ?¡¹‡YQà/@ÖR²o@‹s'ÿÝñ»+5q¿æe ó$¿ã'åcË,¿Ù(•M¸"NAGNbll?ïù	¤¢ï?Akï‰?/'Mâs¨*?&mt6öâ?Dšiºkñ?<‹;ý'Cã?ï­OÚïá`?'ÍRg+·W?pS"~	3È?p¡¦ªŽ?y~óX°N?$˜¿Ë?ïW
Oz+?à?‡µ¯?~e"µÛ¼?o)œ½+?‹
îB(ɗ?wwÛêG?ï.G£ØŒÉ?³šsI¨ß?k™OqØ4Š?h•×©²Þê?–Ãá˜k.=?ŽO'ÎÛ?ïü³&Þf'?/xAß÷È?$\Cˆ_?ÞÀ§â@?0cÿQÀ‰Ó?'ÎHZ{?ïä0y£¾?f§eo¨?XŽ*j)Æû?Vÿï_Ûõ?_âŽX?_Pqˊ©?︪Ë	?iwÒdª?l☊֫C?Y\VQSÛ?u9NH—g?cÎÆ
1¥s?ï×#Œï^•?m€ÛùÁ¥?Q²ý»{šl?B@=	kG?pyýôïJ?k:íӶؐAGN3FGL J1104.4+3812@fzv@c^@PB7¿õMõÀ5®à×E̓À9²‹-Æè¿àµƒíñF@æbu+?üX¥€'œR¿×Dû]õ¿Ýn(#¤¿×ÌæäŒBT¿ÔZ½#AGNBLL?ì$…ߎ¬'?Á=WóË®?R«o¿J?Wj1Â4[?¾"ÆW#
²?Á4ÆÕDž?ïǛèë¼?|	ŒVŸ"â?h<òˆõL?m;FÚßO?p¾×ùG?rŽÞÈ'l›?èm=ÉAÛu?±ºe•­»?•£"©¦¾,?"õ¢˜–›U?˖–f֛$?±oC6+?œ"Á¬?'^±Q¡QW>îQ¦†í?Fø¤V÷N?ŒÉÕÂ+îw?']E{@Zg?éa%LÅ^?ʝЀ5šl?gӟˆFº?oá†5@V?Ê Ðß?ʚŠ<Pà?ïëŽß‰ñ?bur¤^'æ?R·±®•(?R"Ȩ"›?W0¦Wö?W;يIi?æÈÓC"L?µ$s"Š}m?œ½ª2'¡X?–wÕ%k1m?Т~Ö°âr?´ˆ}¼"&…?ïÒøïÚ1Ô?sºLƚí >×ßKB>ðK'HÖÌî?v}<aNá?sº?«{RAGN3FGL J1105.2-6113@r(ßÒc¿îðÉ'ÀÀ7å8ÇǪÀ:)óð?âö''ž!á@7Ý¢@v;Ÿ"X¸¿äƒAy$·£¿èbz–ý˜¿ííÃ3é3¿ÖÜßb]áPSRPSR?–Úö`bùò?ž78´-m?©"9X"c?²¯Ž5ëÖ?í°ä¼'§»?¶!¶ԍ?½×lgK,"?Âv>öŠáE?³7†¥DIe?­²œýì?éÞ!ž`RÑ?Å®Om?bZ?¼Ò3·^ô?§(`
µ3ú?ʙպÃF?µ1ÊÉl?åßXòñ?¸¡­Ü"
?ÐÍfŒ·?ÀՇpøÇ?"d%üCÕ?—Ûƒ¿È?æöR$:?Áõ£…¬?œvÝ-ÍU¤?¢V"M<0Î?Å ÷j†ç?©@üë½i?î. ñ½ü?°ÆУ"?ËïÕ%
ü]?Ð<ºQ[M•?µiYǃA?«€ê§ýUC?æVߓV'?ÐgÅàä¾?ÉJ½€ F?°4Ïdö‡ƒ?ÊÖÿo)Ñ?±n¸<ÄlÜ?â÷Ú/z?µJè#Zò?Ù.F~-q?ÀI¼Pl˜É?"Aƒ±dŒS?†5gã5'T?ââ\¿QAÅ?Àr?‰•ëOTHER3FGL J1105.9+2814@i¢ß"xî@P«à"'À9¾‡«ÚÀ;Á¹žòžî¿Úãå¹þ@¹F–<lî@¼¾@Bo¿ç7âR1Œ¿ã_¾«e¸°¿ç½®J;ô‰¿é—ùUŽIQAGNfsrq?ïøÇȽ.Û?G{,Ò;îk?C§à/Äê?CǃoΗà?3†h\cº?3Ø\ëmí³?ï¹âu'¸¶?†àYj¬% ?pGýPho?ûjÐF"?r}O Ћ?uè4°¬?îÆü
I|m?':©óÝG?'ÅmÀŸXP?‰Å[G`?"[ýR?‡´1Ù–¶?ïÌÌëoi?w¢'zê>'?S¥Wõ4u?V>k½iµ­?uÒ±‹Nb?uà§>3Â?ïücé¼û&?8DmæÍ?5
ÀuË£?4òʪõ§?BdÀ!? .¯ˆPž>?ïæS™Z. ?dî7"‰u?WvZ©¢Ò?U4Q©0‰Œ?[âr?©^l?[îa:nš?ïk=–—X?'ßhË8¦?"2ÙÁ?~O¼nñPk?€þ
K"ìG?v$DÐ6?ï÷¤Ÿx^?U[4Û´.6?$eòj!?*t j§3›?LTap+²?T·¯x\¹AGN3FGL J1106.4-3643@qˆvŸÏ=À@5‡Fÿ˜ÑóÀ9e‹rXÀ;¡6Ç<j¿òñî»ÚŒ@‹U@¤4þ@V)«0ñ¿äÈé˜+ý¬¿äþÍGñÜ&¿×ä&íÌîþ¿ì1 x½ÎOAGNbcu?ï£là¼Â?‡8ª7îÑ&?'K쫳y?…ïßyâ??cf·®P_'?^š™"&@C?ïksDV'T?"ˆ~TžÜ²?}5ÖX>=ÿ?wñVu~Æ}?†ˆC¹pØ
?ûdpài?í¿*«Wå£? ?)s‡ZT?¦éºD93á?˜Ð¬²#t?šG6iyî?â9 ©'?îõ×Ýn}?"{«ÞDãB?c"Dõé«Ê?lü°ö©Ò?žà»¯'§7?"@Š&?ï×úÂU÷?n#ïǙIL?oJ5°GzM?jcQ{û%‰?Qv?J¾?KÑCtp'8?ïÎíŠמ?wo¶¸ð?e¼#"?_Š90£ñ?kòºÿ×?rwÍ)[ž'?ï6n" —?'2±&9a?"PÑPUˆ?Œyyé{V?†Á°nZA?~2—£;%?ïÌØÎQ¡?l &³Re?:È`Œ?6ÝÃÜu?xHßJÁ?k†¾±eBAGN3FGL J1107.4-4447@qÃN?þó'@,‰9¡}ãÀ8ÉÔCédÀ;bŠ÷??åÕè K‹@…B(o@¶@ @&¿åݚ?½¿êõ†ÿ'å¿âK>}ý¿ïÿÛ*f8¢AGNfsrq?ïóٖT[?`\À8×oc?!">Š­¿?CU8~û³?Vq™íöÂ?`&Vìvçb?îÓk¡Ûÿ½?¡«ì"‹w?†ý£ü–`w?£ü¶i/?š¹Çì¦"?žÀ«MÃy´?îÀXYÍ?™ñÏx"4'?›	Zp¶'?ŒZ(,©]/? ÿHòxˆ?"~Ž=}?î:óز6? yԄ႐?Œ*ˆU(ÅT?‡¼ÊúyS4?¥F m*GI?Hcnë?ïüPX?@ÅÀí}`
?–§Ô$À?ây鶦?6Õê*Ê9»??NM­òŠ?ï'XÌd?Œo{FÔB?xzæ‹DÙ,?pÿl^±fï?ƒþè;~‰?‡Šž'h,?îñ|Òʤ?‹o4ėnþ?'É$Ãü)?€jVXyÛ8?+¡ª›[?"šÿ>Fß#?ïŒc i_ž?zzz!ˆ««?wÓ^~ëäY?faZA?€ýˆœ">w?w'ñ†ùÚ{AGN3FGL J1107.5+0223@o«àe0@Kv 8ðÀ:(¯K²†À;´p'I¿Ë";ϗŠÿ@tRY«î@¿à߃ü¬ìæ¿åá̧ý¤¿çN±Š"±¿¼
-Ux­fAGNbll?ïó¤usR;?OmFÿ¢?DñÃûF?C­‰È 9Ð?L|eËM…ö?C.\@"
?ïµ1¿âûÛ?ˆa?'nQ9?pè*/+LA?'8
?à?t~õþó.A?zpíÈ)ØÌ?ïãÿ»¯?‰†Wyaá_?‡N`ç*?{°}¬Fì?'Öswm‹#?¢¹«¬?ï_Y)ù	?‰ül¦2¦?Wì½ïÌä?^½6œ"3Ë?'Ÿ	á.
?‰•zÖ(ùÆ?ïû®]\7Ë?6ðŒ	!c?-ýP—M)n?*F#Uòd?3Žmm£õ?,|@Ekc§?ïä×!¢Æ?g¶#
™¨‡?WJ.ÿt¥?TÙuDU:‰?_.º‰°Ø?b·¼ÀsL?ï•Kݑc?sñ.år'?y
^á?l¡ð¢äJ?|PbŸÛ¸?epx€÷¹™?ïää"	~ü?a¬"q?8|A#Ë´?4_ü­êÂ?hä¨Ì=Œ?`Ûw«wXwAGN3FGL J1107.8+1502@mIÎ ‰ãC@Oˆa .QÀ9®JGKîìÀ;«å3Ëßg?ч–u*'@"þ¾·`T?ÿÙGŸP覿á
/±|¿àVY/"Þ¿Ó‡Twüeí¿äþw}¶^AGNbll?ïõ"\N=-?N$3¤n§å?D	§<¹»%?@ACËãº?Eäæô<9¯?Bೄ'+?ïFãNnx?Ø\ð=a­?†Ç¤]±¥Ä?'~£àÁZ?‡ˆÿ-|?ˆŸÊsϖ?ïEÄd]Ë?'\P€#y?'6xÒ¿?uöpo#X?ŒXä~·n€?w?¢r}@^?íî}|"C?™sú?ûc?"^Ş?‰#–»¡^è?§©"ü?•âAÁ$ÿ½?ïû̲©=¯?4RŽñÏóÝ?0»ŸãÈ_?,ZÚ6ýñ?1†®Ý?&J±5"U?ïÅìÑ؂ì?rÂ9Ÿw{?mv°]ßÚ?dT=(ÞPB?lœ}áċú?l°€Ý~T~?ï¢ãI»àÁ?ròbö~ÓÄ?u*CÏ·j?lӁҝP?ydõq´?bÅs¼a,?ïf€Ô•‡Ö?xš£32è?ƒuÍd\Øì?kaÐx¢?'éý"¯†?r&U‡‰RAGN3FGL J1109.4+2411@jÏu@‰]@P·þ¿ù³À:\ø³¥À;ՎñŸêì¿ëœMÑD*Ò@
œ¯ê"Ý?þ0§á6¼?ÏQ–íå¿æŒâaÖ׿ßÐïì·xÓ¿ ­Ð¬*AGNbll?ïì¦(j¤±?_Ùö."•?2
úRÂ|?1|»ã+?aušd¬?]R†‹¦?{ø!Aø?€­Mc´¨?kHq¤®-Ï?pp)®†-?sËJ½i?w+gҗ%?îñ
¨¿@6?…×%ܬ•?ˆ¬™Ï?0?wâ5Ï?•ˆ£#Ç_™?~¡Å 8O?ï¨æÛC¢?€å/Y0á0?0šªQÖï?9œš	҈}?…BO;ïÇ?€Éø¡_?ïù´'9J?>Àé*<W?$ӝ2±?m¤à|Ì?D+ÆuµíQ?:éòÒæÜ?ïç;džÔÜ?d·?ê7?Vµg»†?Vï)¯V
a?[…¯Ñ$?Yù¢-êÜ?ï€ô!®<?tµ"qjV°?zþzËI~G?lìÍd˜;?'Cº.*…ô?izúï‹BÞ?ïôÏ	ND?S?tÒíO³?a§0¦?
ÖàüÒ¿/?V¼GC‹p?S	Ÿ«tj
AGN3FGL J1109.4-4815@qß%¿­)™@&r¬azŠÀ9¥—­[îÀ;z÷Zï:?æbÈ
í Ï@_Kä/@ôÖ ˆ‹ª¿ç8äl?ˆ¿æuºIðí¿ég#™Ñ烿çÌñZAGNbcu?î¤;lc?¦ÝaT	À¿?Šæôì%­?}±g³ÆÖ?žÈ1É?¢ýXWpYx?ê5î0l%å?ɺ"¾‹?²ZœÝàŠ3?µÓŒ'´ã?»õñž¾F¢?Á¼ÿ ð·?ìtF×æíq?£<""? ûÃ	†?…G¹8Vš?³à:]Œ»? =S‡6w?ä
IàÚÜì?µ~ÈclÈ?ÇUîÛ%¼?´¨!°âˆ?È·'¹f"?®®Æ݌?ï¢Ç•!Ý?'Wǹ¨ÝÎ?e–noµ÷Ÿ?kœHËê?èºÄX?ÓFþ0
ù?íÔy%Ó¼?¼^ðïI'? 
Åâ,B?²ù%«—:G?¢ªÜÞ£õú?­rß]­Œ?îÃ磒Á¹?Xé  ¤?Œ"‹ÇÔ'{?|¶?´R¾?™qŦN$?Š‰ÄžÜÍÂ?ë—Y(e?]ìÂä0?´('µó¸?–V.%ð|?¯µkKm™?'i60gXAGN3FGL J1109.6+3734@fµ'Ì÷@P>àŸ°À:ٟâˆö´À;íܜM©?ىƒ•þ@
ËØ:&—?ú^Çá?â
¶?äê?ïø̜§h¿ÌŽCE鳿̸@	¹ŒAGNbll?ïñzWÍ?[KÓà·?EÎÛ¢­y?KÿaÏÓ?R#XX1sƒ?UV\×?ï>™¬ É?¢ð;×X?ŠPÿ³/Ý?œ…æ‹6"?†•9ˆmê?ŒY›8y?"EqÏ?'Ií‰Û¶u?'ûNÀ«¢?†g¶¹Kˆ?—k-¸"r?†@ÌPt?ìú–b
6?²mã[¶ƒ?²EéiÀ?±!Y7›ü	?˜"'îJ:?—°¼fqOÙ?ïøkD$OÉ?I˜"ºº·?4®¡ï?5˜á~5ø?CûæAVâÎ?CI€¼zÝ}?ïʋ ÌW¡?y˜€ø2‹(?i¾Ö…`r?nyCžGw?kµˆ{LÇ?nèð|ðã?ï;Ê´³j?Šs¦Ýþ7?ˆ»k«"¤à?"~Sk½?ˆd!´ýð~?}["_®?ß?ïA~ÎÎ?û?‡O=ãŒî?'dÂà*pÄ?ÄË)<B?u­Œõ*;Î?tsyy`cAGN3FGL J1110.0+7134@`µJ`"@E°…ߨq¤À:P­'tâ*À<î
46h?â¸D{"@ƒ`ݐio@>îÿ|¢h¿ã5~VƒV¿ä¿ß"ƒ7á¿Ñú,›-\¿äDŠã76AGNbll?ïïÓÛ:#?_̌ôç;m?Cò´¨è´?H0dײ?V`ÜLfFñ?V®üÊnã2?ï1|´RúÆ?•DÚd4ê?ŠÂ1"K?Š½=@?‰Î6Î+?ŽiÉû¿²?ïå>øR&?'šènÖÜÍ?'ƒþpÁ…²?Ž‡Š u?Œ¾³j·?-?x1ˆÔöu?îšދ3?›`¸tu7?'p+~an€?'©îñýÃA?›L16%9?'?²·;¯È?ïûOÀmÕ?<l{xV
À?"ÏÜ_Iÿ{?!-ÛÚÐÌ|?<"v~?6_äLòèÍ?ïÃ]wÕN§?s¯È"*âP?nýqðã?f7"ðÛEq?m¥vØ]©p?j]Ïò!Â1?ï}wñÛX?ƒŸÐ¤Ð?ƒJ9Ñß8'?'´Û'‡Û1?z¯ÌC2?_'- 0fl?ï'KÚE†?zzÂ2ÿ?ƒEFøä5%?r·@·Ê?pOñÂe?hMþ]
¢AGN3FGL J1110.4-1835@q6_Ø­¬@CȾâ(À9Pc¥ÁÆ	À;uéÀ"š_?å'ÎÕÌ@x^áaÚ@)? ~æ?žÞ¤Kàdj¿ãzuNX¿Þ¦¤*Ru)¿Þ÷Aö¢>AGNbll?ïë+ÉÇ®?Y+—ÏÂ?Tj÷Öû?OAFÿ{q?U=v9Œx}?MAö°g?ï1ívC0à?ŸE–'Ã?:?‡ì±Õ¶¼{?×;RËÛ´?‹—ðª«y?•Wà5P?ï "ÏIB®?‡•xk¯M ?‰&ÊúL¨H?}m£Sï?Ž´)ØL?|•ÁPÍb?ì._ο½?¤ÈÜZù®?›Í àØ?"¦èƒä0?·™™gYP_?£)ïŽSüh?ï÷XÀF½»?R`zªæ%?E%¥C_DÎ?Pàµ&£
?:ŷâ?2%nû›T?ïº8ä*¿û?"˜ß1Î]?rM€<ف?|¥ÝQ™?pÈ@_di4?v¨öŠ\¤?ï"SUUš?sh»æ?{GžÛfi?pÙ-ò™H?zŽ¶FbŒÕ?`Vw.­`û?îÕûªZÜð?‡_óõI‡w?ŽXü6"?tåÿ¹B?–žÁC#?ƒX2%'AGN3FGL J1111.9-6058@r2iŸ¡—¿Ù<ޟªw/À7æ>)0zòÀ9ôúWI'ñ?ú…aêhi@0{âN"8?ü}¶¬¤ä&?ïÿ‡¨3¿áÈ%Qâ傿å<"Qw°ª¿êý~ñL³ãPSRPSR?‹°9cɏ?›"ÄZœàt?ÚK9
÷H?ÑF5·zˆ»?âk¢•8-e?Ñ8ôSàŽ?ƒ‰~8Ö
{?µ(& äÎ?ÇϋŸl'­?¿cÖü?é½÷ÂÏ.?À‹ôÍ>Y#?§Ç,Þ?˜ÖLÛÙb»?׬/³ÌË ?»w`‰­"?â¸;´rI/?ºÐ+P³?®ÖdƒÀÇä?¤E…lÒ?ÇlÂvÂg?µ9À>ר´?è7iBBè?¸š¡ê©Š0?˜Õ"£µžª?¦ö
§¢4¸?Ü8òR êN?Ò?`Üti?áÚ±'Ýã?Ñû"Ycž‹?•ñi‹Ë)þ?¥›¾¯J?ÒC–á6?À±ÁC+λ?æé'ÿqe?Ìæ‹md?·!MûE"?¤Öt~G¨?Õz9ãë;?³tIGl‡/?â^Ð#)¶ï?³ozS†¤o?²ÄG¹šCw?¨_šR"Íå?Ìпds5ñ?°¼•‹n½á?æsG0ݔ?´Üž"ê®OTHER3FGL J1111.9-6038@r0Žàm"¿¶nŸËùÀ74éœlÀ:Í<^U @Veòùg@¿lÛËmQ?û'ýXZßõ¿àÍD@÷–û¿àŸ|Ò¹uØ¿ã@Pó7š¡¿èŒZ{v™OTHERspp?k3F&u?bíün7W?ӄj°…/?Ì	IÆ®¶È?æ"—™†›²?Ì	E4MË¡?Bîê²,iž?Wÿ¢³Ûу?áÄÆûÉÜÐ?Á'ó'n.Ý?Ülú'‹f?ÁÇ.ZäÜ?±À	,êé?Ÿ™jš‰ ×?ÔPÊ#`h‡?¸†üv:X?ã³Âí¥àO?¹•J£&.?]ø!Çøh?†ˆŽ%êl½?ޗ?ú?¸XQBbä?à1p»Sþ…?¹KZpÃk?o$ùØÓ ?n¬9Â4ª?ØÊ£Zk9?ÎV™Pà?ã{‰Y–°l?Î$U¡êmi?\@½óˆ¨Ò?psÝÞõÈ?äO‰¡î–?·øçlÕ#/?×D«þBˆ?¸CIȌPz?»ÓGmÛ?¥n¼ƒûãì?Øï^¥°\?´yÌø":Š?à"HD:?µRc¨ó‰?"¯¿y;Ðó?‰›"˜?â´Ó÷ü?³MÊ(Ѳ?Ù[\Ô<?´‹ë,ú®MIXED3FGL J1112.4+3449@gZã`'@Pàg@™ÅÀ8ðùÏ5]À;­Ôèë?ôÉ5M¿¦t@v˜¼¤áv@Á»=iè¿Ü €±žÒ¿æ·¶Õê'À¿éÇRºb¿ç6–ŒkU0AGNfsrq?ïøÝ`]?Cã†Rž¨Ê?@™qÕfW?=×õ¥Kg?>¤VYh¸?6K'Z&ñ?ïƒ.ç&ÈÊ?Šs­.žd_?k=ìlËÀ?&mÚ#yŽ?~ýN`'gM?nß¾bm?îè…ÿ6n?'"ZC4¶?'Hæ#
ù?‡çP!N°ò?¦|}•\<?…=1g?Ð?îgx†hS??¡fúª¾u•?œ¯,eÕ?"³á›`?–aÂÉ°æý?šo=›.(¹?ïü6R;P?2×õ;
?4×Þ`sö?-MŽ:ëÊä?%,Þh\
è?8ل7?ïÏ_Ì÷Ȃ?sù(®ô?gñwÚâ¤!?f'*ٜºÈ?h®»QÊ?i={^Tþ?ïX·ê›?'ŸØõö?‰*'Ь¾*?¾ßÿ[¢?€ÏDÒ¤ž?l®Ç-?ï &DH•?yx¶úmd?')*zÐû?o![ræ~?g5³ÊZ÷?mԞ£Ô»ñAGN3FGL J1112.6+1749@l¿VÀÖõE@PZßÎ1QÀ:×ï¤h)µÀ;Òÿ¬óéq?âº_ð*Ÿç@ó×QÑ?÷x‰ ¥'õ¿í-?ö‡~¿àåñ!ö¿Í`E|®HË¿³"‹RYBAGNbll?ïâ<Ž|?pÕ>}sñ?E³ ͬ[?IN@#·bS?hW"2{C•?p0?
"Ú?ï©qÐÆU?ÅüÈßÄ?t`ìYàý?…S&\yí?væ+ѓ¨¸?|g獏Â?î´¤s¬
ÿ?"å¶n4¾?•è-.>3?e›Æ?"ƒDm˜3é?'È]Ó÷?ïƒuÿì?—nz ÉÓb?r×]?8^?†Gýܶ»?˜¹ºÚÏ?"¿ÊÝi?ïî@iÉê'?dX@‰Œ?5•(`)?4ÿö0_18?^â3ü-Ñ?c©S€B¡?ïã•ø'ç?j½ÄΨþg?\RÎgÿ³?a6Ú>pÅ7?]Qǟóš?["àý–Ñ6?ø?"= a™Sø?"cZpÎo?'½WÜ?‡'â®?H'­üƒó?ïÆÆuÅ©î?uûŠqzÅ?hºyØòì?j(Aiêî?p?ˆsÂë?j>î¸d÷ÛAGN3FGL J1117.0+2014@l2؈v\@P×°`À8œnØû¯8À;"pdìêÀi·|¯Þ@=oxˆÒÍ?ýÝÎg¿Ø£f^P9Ì¿Ý,éo<EM¿Û•7	V•ä¿ÚžoP^«÷AGNbll?ïþ=‡
ê"?&âÀ—ÈÔ?
ƒ}ø¬3?øÁX²Lw?$ꁈdO?#~Ž–6ñg?ïÅK}p²ß?|!ÖýC´?hC¸I±?j´àºýó?qJŸq±?s©±-KÊÿ?ïYópœíƒ?…EÛªõ²?~Ô>›7@?w¹Çà÷uœ?Š~õ•?€ºÒڜ?ïÁeã+*s?|¡¿±œ÷È>ÿ²"o^ˆ?
"vTb?-\aÜ:<?|šûVh?ïü؏	?hj|è·M¯?	—X°Ò?Çf§Š/1?5ÚR·¢,T?hcݲ9®æ?ïêËrړ	?c
YmU(1?S@üÿUoM?Sêe¢8Ôÿ?W('~>Y?WÄ8àŽy?ï¤îUòP?wôÖ*•g?uEOm6h?q¢§ìŒëi?xC†ÌO?oHêv·0?ïòFg~¥‰?Tmí‹4¯;>̪‹ŠƒÛ'>×A׆A#Û?[dÛXúË?Ti'Æ6ʳAGN3FGL J1117.3+2546@jgžÿŸ‡ð@Q:þßÙïËÀ:']æe$GÀ<
µùK°Ø¿ä…–À l@
]zž,@,Ù¿úVs¿é&•‹Bõ¿ÃÑ9æM¿å(©òçz¿êaÃ$#îAGNbll?îåwp¤Ø½?˜¨œIÙ]?Ì
'ÃD@?–àžRöMù?vJyL§?wñ"ܶD?ﻣ§? ¼t"Ì?'=	$?•/ølíüä?!­0v×?'aܚÉe&?ìˆm°»'?£ˆÊ[é¥?²"´µo? ŒA˜*øŠ?£;—»àûµ?Tñgïz?îƱTÌ?¢–‹AC?£¾|yŽ'r? "¡ºD?–€Ž6¸C–?ë}x7Š?ïŠÓ‹S?…™ÈŒi?‰l«z'?"I»Ÿx·¿?`ο2àÈò?\¢ä¥íI?ïÆîMô?z	äãÎ?mªã½¯ñp?pJÔ9¨˜:?l=.)v*†?o–ÙõL]?îC¥¨Šg?—
µ»Ž6?£Âz€"?"lô;S'?Iù²Ù¾?}Ç£`é£?ï»)ë6'?qà8¤^1?q@.ß(?h¬œ£\º?q[6b£Ù?g³5NyáGAGN3FGL J1117.7-4632@qéî@…+N@*¯a	/TÀ9…oîMPÀ;tÿ^Ë?õ{ât(ñ¼@ÁQ&
ZÜ@qA%iǿѱg
üx¿ë2ÉlCÉ¿è…î)qq¿ÖÏ,;OêØAGNfsrq?î±à¯¥?»¤Ù­t±?­KŸˆ?§ý¶ŒŠ
²? dO5ê•?µÆÿjo9¾?nÄXà?±‰¢¹O'Ï?Š.TÃ?'`ÏêÆ? 
ÌÕ?¬/ï»Gõ?ë̾—ãæ?©\yEĸà?±C†¤Š¾~?ž•ó™U¬#?°V"žš;S?¡ÉܱÜ?ê`)Çdb?µÏ;"´?®ûU˜°?±¦Xû¶ô?½ü£ÌoÒ?®ÞóÛxnù?îð½øs™«?ÁæȖ:?'|}n€??˜±£W†ÅD?˜ª,?À'B:@U?ïlDíxq‰?›
*ZÓ}n?v]"(–?|©`u}?‰åÓWԞ?•Ý}Ù{…?îd/2,?šc·iÌ?¢%­…&‹?"81{¡V¿?—ȱm?}|$há?î(Šùà×? :aysˆ?¡{$l#?š3í)YX?˜¿Æ3Ïä?‹ãÿA´ÃPAGN3FGL J1117.9+5355@b¦²_c<æ@MÑ?ùSÀ9ŠKn"['À;µ?Cä?èY²òÂ;
@¾Æ/ú™?þâà?Ee:¿ãTö0À´ˆ¿Û¹Ò;C}¿Ü|¸¦²Ì¿ÜdŽ="¨ÕAGNbll?ïä1
—'4?uæ~c`£?[îU;¦^K?oš	28v?[¯•«4¸û?`Wևáã?ï_÷Þ½
?•ÜaÝn?"ªv>«K?`ƒO4®?ƒë^
ù|&?‡ºpêþÚõ?ï;êñóDR?"®ˆ£ƒüo?ƒ¸*?wñÊ?we_¨©!?MSÝ#'?|Í®'¨Õ?íÅÚ£¶9I?ž¿Ddcî?œ=S¿èX?•@ƒeÁ?¥ƒ«å"PH?•Ð'Åøºj?ïö#­Úe?f h%'?A]M¦
?RÁá0æä?FúNكÂ?]Ù3ȏgp?ïÌʸg™?vŸÎ㺑l?h¹D(©ºu?hOBmðÁÇ?j|ªòó­*?o&î¦nBÄ?ïŸ]²|ƒM?tX¾˜6¯?u`ò&'.œ?gm<ù«‰?zð4˜|zÝ?olõÚ¶½?ïQ::ð}?'Ÿ'¹Iòñ?‹~'¾®þ?vP''9"?€3R#¤A?vOÿÔAGN3FGL J1118.2-0411@p{1\1@I·ª RÀ93_?*¸:À;ˆüàÎð?ò_9ßÞè@™+û[€"@…è j¿ã1Ró9j|¿é–žN¸ä¿è_x՘'!¿ïølD"@AGNagn?ï÷ºÝ>½‰?Jl¾ççØð?B&€»Þ?A Þ"×kß?=êÓù'¯?9\?d°?ï©«<%Â?Š=NçŒ?tnÝ%† ?ƒÒÖé°?v»"Þöä?|‹É£;?î\Ûã¡›?•®ÛVD³£?¡4þP²²á?'Eÿú²ÊS?'ú‡åžÈ?'³WO"?ï»æ¡æ?€d>Ik¡?fÞÂRtf?lmÐp6?vŸ â=Ã?|D7d¾$?ï÷ÇÆÂ`|?Gþ¶¾ãŒA?HZPT"?Dç©^ғ?1
*¼"R?),*°–?ïàÌf?k ",eˆ?]Üç	ل?Zuàþò1¶?`ó¿Øƒv?bIáçÀá?îì^^ÉÓ¸?ˆñÁnŒßÿ?–ÿ;³%N?ƒ®:÷ˆôA?†éòã7W?uóA¶BĎ?ïï^Ž|?_¹׀3‡?QÏ(›Á[?Iˆ]ö֟:?NçvÙV™?ZhšsAGN3FGL J1119.1-6127@rBTߋr¿áVnßå6À70ˆzdØÀ:I=tՔò?ꦥ3‰Lù@ŽzóXh@ßÆ´{G¿Ý"û10›÷¿å-æ‹Ý¿åÆFª0¿è–Ý
Bà6PSRPSR?¹G¨È"?¼°V4.¶?´½ËÏû.?´È2¨™¾?ê?Ql·ÁÖ?Âp]DB"è?ˆ¾è&¨1ù?˜g³ÍµE–?ÇèD#½Á¹?¾O¿¨Cwñ?é¢óVh0Z?ÀxJ°·?ÄeÒ	]Ä?¯('ŒB
j?Æ;>
Ê?±ªµøÂ@y?åWËi±…°?¶.ó´µWO?Á7ð&™ð?°$W1Æõ¾?Ä^©ˆ;?³p½g¶ô?汬L–õ?¹ž½°Ò?Á×lm¼q
?øµç`ªm?¦bK]MBf?©ž<ž·~?ê$.'ÔG?ō{Bv? ‡tOHd?¯š¬ &]"?ΒB}?¾c>˜Â?çS»"‹Û?Ãy'c€X?Òw|†ÁÙ1?·-ˆ#{?Ƙ]©±ó?°[Û6á­?ád«6‹?·—Âýž¯a?Íu¥Ò½Û?³vÔT4óm?¼ºœÉyÜ?¤Ø6-%·|?åBòK•?¶Yk pOTHER3FGL J1119.7-3046@qŠA [À@<J€VÒuÀ:¼*JVegÀ;ÔËÔI¿×)»9t@"e²â?ü?ø¡, qúï?ÕQ{ˆ6šÇ¿è3Ñ\î1e?é
bh™¶9¿Ï€Œí¹¬_AGNbll?ïðSµ½DL?\ƒ–¿ ?+íe˜f
ò?*øÉä)??[Úè£uÎ?[³Þ´>Ø?ï³Üi´
?ƒw·'@{?n K[¿_¤?o"ZUƒ	 ?wmìg@?}4`†/àê?îæPÖԄô?Š6ÑúéR°?ˆgàò›(ë?|Ç}—ÚK–?—ô±I6ö?ƒ·•uûU?ïp/ªˆÖ?—ß²áìÎ?!s®ÒIßK?<þLâáÖ?'×#[Ýrù?—ÇÇJ
I?ïùów—¢Z?>I%þW"¨?"ˆ×¼S?ˆ0ÊîT»?CêØÝØ?;£9+I?ïå8Þʹ?dø©déÌ?Wa¹?¦<?Sez¾š'‡?^,Š[eçÈ?^n¢š1?ïoü–˜'?|g½h%ºA?zƒ=Š@µy?m0õkL)?†¿\õ?x{Ɂ–&?ïëZX)üm?eÑA@‡®?#Ì,õþe{?9'CißÅÇ?chäÙՒ"?d|©ÕĶAGN3FGL J1120.8+4212@dúë__(@PŠ¿Ý/ñÀ8Ç¿ÝÑÀ;øãú?ÖNL¿ g@ÿyZ3þ	?ùܒÉ仿â_qü¶cC¿Ôô¬'Ýóï¿ÎÃÕÍ|u¿ÇG¶Üå7—AGNbll?î²÷ô˜Ã±?§«ê
¬9O?lÉ«Øÿì¥?oØÃĜî?£åöf­?§Mᔗí–?ïy"¹…¿?"ãé*Ùû?~TÌØW¼Í?Šä‹^?'ŒëP'‰ñ?‰€3übºÖ?ì%ç¤Ù,›?¥cã`TW?¢¶ÿ8óW?"D+Ð~¸6?µuCâS|?¡qïÇÓ³?ês–+6JÑ?°‡DÍ!vì?15,1·2?''–8¼?Ä+€¬½?°^S¶¸Ç?ïD‰f	Ž
?ŸãÚ&?d¨Eø/?kêÄøñ?"ÙÊ|´ˆ=?ž÷›
Vt?ïÏ+T—‡?yBÙ?gúDW}V?pù›ß}3?hêub;Œ?nÉKî×íÊ?î…KŸ¤?™a¹³‰gš?—Å:%M"ó?ŠpÞu§Þ?¢µ@×Â?'{2…¡/´?íâCÁm?–?–×ñq†zå?‰b"óˆ»?w£ÒxJxü?«ƒ;gÂÙo?•iöP.
AGN3FGL J1121.4-0554@p£Â # –@I9PßìdBÀ8H]®îÀ;NO~ÃT~?ñ¶O)Þ˨@ÌápGæŸ@î"ßu›ã¿à±`²iÁ‡¿æ'þ'o¿ãÀ¥«ºrF¿ìd{йtAGNfsrq?ïéî*ëf?\—œçÉQ¿?bb»›%ý—?Z1b>£?=xÌJ§?6cäåH?ïÁϽºW¢?~v3¨köö?kHTž­ ?n/£,ÿ‹;?qt`w"'?tu?ôC?íþÿ".ו?›^kT¾œ~?¥\>ºò%?–bs$«T.?•g.¢/?ˆt&°}g³?ïéÑúÖlÖ?nwpð.ˆ?5Gœƒ3ÛD?JK8kÀÅñ?c…Ì*u?mÝ) •¸Ã?ïïØ¢î×å?V¯Æ{Ë8?[´/††?T웹³ƒ?2j*ۂ)ü?,œ^Hg×?ïè,T¥Qf?dxÍÚ[†/?VhÀÕf!?Tþhß,?Y>•@Až?Y™ˆ–qÞ?î³¾¦U?"Fùß`•o?œìÀbO8I?]Äö!p?‰^'ߺ0?}«_XñÙÛ?ïûàw¾A^?F4Ž¥#±?òž4ŠS‡? ûN©»Ÿ=?8ÿš)õø÷?D¥³WMAGN3FGL J1123.2-6415@rX'ßüTzÀA¯ó£À8\š1o
ÕÀ:áN_¤?ø&»˜Çâ'@g?A‰b?@å¿ÚËè÷¿ä[[¸ã`ã¿êŒ#0J_¿ëd—iò¸¿áHê¥êzAGNbcu?ïŸs•+©?†'J¢¯z©?R—g;S¸A?TC	ñl¨™?…ëv5ZbŸ?†
܌dP?ä-^ÄÖí?Ó¦ÓF—Ä?ªR⨐´A?µ_•Þ@k?ÔZæ!ÿÑ~?Ñö'Û±¹?ë¸f\€_?©8hPq=¢?¦RDþx?–·|.ž?·å"/£Q?£ô.uIë?íi—K
ÀM?¦#‹òQ?…>|uC?ˆû-£ ?²}×­a´?¥Ì.€ì±?ïÝU?;n?r\$9ä[î?A¡À֐tþ?@·áî·d"?nBP§Î=Î?q'=ð1?ëÌÿBüæ?Èuc?'ÒÚ'C?˜wë©(O?¼ãOg"¯l?Å¢þÃÑÝ?í±™PZ?ž°SGåAÅ?ș̌·9h?'*ì/-?§à(gZàª?–®OÀxb?ï;ø;yà?‰¤X]ß?{Þ[fÂO›?q'µ³+j*?'‰a°L£?‡>'´cy–AGN3FGL J1123.6+7231@`xÀ Ç@EˆßÊÖSÀ; ýŠúaÀ<*%@+i:?ñ_ &P¡®@	†ÁEA?ù~sÝ@
¿ì'‹'nŒƒ¿â ×@n¿á^ȓy'?Á.å»Ü´AGNbll?í"`yß·?À¤'ny}?´;Ï1,Ó?À†x• i?…§Yas›?ˆñp'?ïh,G?™•*f^?ß"Â0?ŽOôubv¥?" :zRÁ?Sã…_ ±?ê''?°Ë([¡ð?¼'ê
d!?¦‡o,€?³aZ|½Æ?£‡pvZ†Q?î-&ÓQÕ?±"ÔÉa£?šªdùñ÷h?­)!å€ü?Ÿ°Úˆ42?ŸO7fAÕ?톩^Õð¯?Á<·
èa?²ñžÑ,|?Á-ï|z$?{|6šæ\«?z8çîâY{?ïÖ'Ço?Ô?u®Ê
kס?d;Ŝ5?g´Š ØÐ*?eœs5#DË?k²d¿?ìÁḻôÚ?£â	Ý¿ÝR?°æ²óè¢? 	5"øªR?¢ÍP€K?"']N ¾?ïį$£×?Ž=¾||þ-?‡9ét'?‹Š4þ¯Ä?q©Õ‰Yd†?sÅy
AGN3FGL J1123.9-3653@qÁY_í¦a@6Â<à[À9
´br»ßÀ;Œ[™ƒÊ$?ÿ>åCJü@X°få'A?úšÚ\ˆ–¿Ñ ˜Å'οÜëYοáZŒÿ_úš¿íZå˜ÞPSRPSR?p‡ˆÓO~?m÷BI'&J?ïÆ@/YÓ?àkCԙ?h°¿c¢M³?wHO{p•?|Ð×ãÊð?_neé\Þ?îaèeéq?³48]ªÛ)?¦Gdà­¾å?²m#'º?¨ °ûe/'?˜ÚNÃò?ìUö"ç^?¤¤Øû?±?öoÞ_F?ø-¶{? Å­¬r¥"?ýkmdÆú?íPB*ë?£–Œsì5ô?ª6(|"&ø?×õÂ0ß?Wx:möèÔ?X‹SRk?ïådÀä¯?i·ÆàŒ¼?]¾EZ)÷?a,†£ú?"Ò{Þ(Üñ?¬Æ‰;Ac?í\;–ÈÈ ?¾#Ÿàc57?°)"QSœÅ?¸Å:ì(÷_?²ã
|¦í? 'š¯‰¿?ë¡âÝTž?¦°°¡ô?°
፸µ ?º¦TtÐ?±æQà'ç?—Ï<%»Ÿ€?ìÍÕ0ª
? 0ëâëî?ž¬û§¯?ŒZUà,1PSR3FGL J1124.1+2337@kDÛ@-¹@Q€%ߙXÀ9ºJ«õ¼°À;ÛjÕ`ð¿ö9ühEä'@W©¯¼EÁ@¬=?üoR¿å(þ§Ê¿è‰.+PU¿ßžo¸…Ô&¿ê®ûC€AGNfsrq?ïå1Ú1~?fe²z{È)?WøbBÔ2?U›Ø×PÃ?]݌WM¯	?a‰z6'Á?ï¬"sÙ|Å?…¥·è—·?qïM®J?wrïÇß¹J?wÿyI·f?zˆ\Í6Ý=?]Ö
Ø?14mjÉ?¢'È'j?´ˆøª}Å?˜¼ÂõzÄV?†òo±ê]?jàɄ?†î€?š8•?Yý
r´q?YßÆ#cP?Š÷¬þ€m?…ÌLG¡í5?ïõéÓ}¸?Lþ׆n?E¹ìÌëÁ?@LáÉR³x?B¡³V»U?Bá~›$9?ïáÕìl`?iÞRÇ}K"?Zôۇñ=ª?YNiϺXz?`¯¥˜­Þ?bϛ‡#+?ïr³t>ÉÈ?{=ɌÓ?€Ôei†—a?pµ-F$?'~½vøº?sJaŠŠ+?ïí߂˜1v?Y5ã,W?,bðdÕ`P?2òJÌß?`ZN˜zóÚ?WߧßDVAGN3FGL J1124.5-5915@r@@ Ç?ü5:ßÏÞÐÀ7ƒ¸µ¾"NÀ:|{üР—@&,§¨Ðï@¨Ù>Ú[@ƚŽ½¿ßل ä¶¿ã}á·aøæ¿é[J÷š¿ëet®/PSRPSR?d?˜T??n›5Š*WÄ?îkÞjV5?¯89ÿÁq?¨‹#Kí?®Œ2ÖP‹?C¥@õž<?[ðÞjÕ ?éàÃ*ÑS´?¹…F¨ëM?Èiq¯Uÿ¢?¹rw't?°¹¥Z…	?¢á	Õм?æb·	8…O?¸D<¯ñJ?ÎQ-w»?´¿ÏãRI?o'¹9?k	kÅ;*?ëè\;Ùä§?¯ú~ù¿¥ñ?¿Àˆ[XÁ7?¯"û1^?W<äÀgm?d¶^…G÷?îÐ=àÇg?ªµ[&xW?¢DÔû']a?ªd®ÒÒ$™?`áØz
á?p$ÎÚH?êm㍮~Ù?²¥Å'ó¾=?Æêfvè¦?²½ZÛA${?ÄÍhlë?«p¶šˆe?å!9³Lj‰?³y"¹I§?Çmeeèñ?­`ãÿö@? sÖüýr?pv#ûä8¸?ënã§Ò
÷?¨F6s™$¶?ÁKmÃ
A˜?§–>À6ÐPSR3FGL J1124.9+4932@c4ú D®†@O /µÐÀ:dpA±{8À;탠Uu¿Õ.Bç
ô=@pG´Iž/?üل`wd¿êÛÆwž5¿Ü‹æ¨b'¿Ó›'Uy¿ÃžN¬'ÍAGNbll?ïýÂ>˜ö?&›ÙT
"g?ÿ'ÆEaÏ?d©¡¾µ¥?$ÜO_ö»o?jzuF°?ï¾ë? ÷?SǼiB?mÏJ<ò?s±Å$VàX?r	åZ¯óQ?t:£
Úa?ï`úL‰-?'ÿø™?"—5®f	?öøòP?ƒ*7ZŽ½?mùE]ГG?ïÞ,$dýõ?jë>¨ã^?&ꐛ©?,}£V¶Ä?p95>î)?iÁQY¸Ó?ïþ±…bnÏ?¥ãŽPª?9'·0?
¨Kõ# ?•Êc[´?
"ÜqçJ?ïèz™½ð€?cڕ¬áà.?UÉV†Û?UAY°Û2¡?YAuÀÊS¬?Z 7q?ï©adì5??y<…â@ž?v­¦ãqÐ?uÄ ña2ž?t¡¦­¥&'?h ×È»0?ïúÎìü[õ??úƒêAv¯?"ÿ¡'?zJ'6V?BSÉ\ÌH4?>)׌Ù-!AGN3FGL J1125.0-2101@qT%à.©a@BÀy`>.9À9øŠ(Ž"À;"ýs]Å®¿'½É;²Y@
÷áíEh??üŒ»à@r¿ï`ó˜ÇZ?é<Õõ"@¿â8Îò'5Š¿ÆÿxñƒeAGNbcu?ïÓgÇ3×?weӛl,?Pr®ß)-d?Kcžc7¿û?r/p¸|AE?u³d€¼Ã?ïrnšÅò?"y­‡5Š?}"O",›¯?†¾yØp?"¢1ÈÃáh?Žqæ»û7?îÊnä\å?8…iÔË?Š/g¨"
Ù?xv»€™¢d?™šo¯Æk?‡£`oÂ?îó»ñÞ)A?•026ƒÖ¬?‹)4†äC?ŠÈ¢h·?"óç…ð b?"g¢3m¬?ïæ· µy–?Š4›ã×Ȃ?:­©dŒè¼?@p9–½?eó*a)ôò?ŠÛo"òÈ?ïפT'/p?p1p˜‹€?aüžù?\==€Að?f_
IL?iAòg]Ö¤?ïsN·•z?€˜•ˆW4?zØ~‡²?p-«5Bj?…Ìäû5‰?{§Oz¿¡Z?ïÈé$˜w?mWéb½	?d¶˜ñ9¦Ý?XÄڟz,?q00"³Xð?gè´JÿŠAGN3FGL J1125.3-5824@r=y?ò^W@Î0àµÃÀ8ôËá©ÔÀ:§TÚLè?ñ¬·xÒ¤¨@
ÆG²œ@‡_ZX'?í´…hñ¿æ[›l-¿ßìÅÇ¿íV" ÞÇÌPSRPSR?¨IÁ'6G?¦äèª@?ߍ+³HS?Ï~äx?ÝáO;ã—%?ϊŒ§Sý"?½Øý‹ö1º?Ãl½&«TF?×p{¦r"»?Å&m½.?àŒ¢z¾¸?ȑýÍ¡?Ë[pi§‹?¬D¯Íܘý?էϱrm?³¤Ög3?ܪxþ??µg 3åÖK?»w¶¸ìΨ?© ¡Dº˜b?Ò]N¥)š®?¾&{ل ?ãbaÖM˜Ô?À^ï¨ÞŸÍ?´&ÀR"ß?±}G‹¿BI?à¨Tñ&¦æ?Í]æ1š#O?Ù¥¦	`ô.?̆Ç3IG?͗h¿è?Ï!•ØU'`?×Õ O/,?ÅX?5ŽÆò?Ù^«ªpßð?Æébjêk?ۄcl`üD?³¶‹	6t?ÒÈ€à˜º)?°âåã«(?ѳ³I"?±"<q<²?Èf‹zGî?±•»`æ5.?Õ#ÀÔÆì8?µ
ö»úÓ?Þ¨ùn‡Q?¹.p\²©"MIXED3FGL J1125.5-3558@qÀ» 1ί@7»'ÿùJÀ9LPtTfÀ;ZHþv"?Óɯ
@§²@h"qM?þ"tÿ±Pš¿Â¦¹r|õ¿Ú·µìêD¿ÚÈoT†¿ÙZÝsZAGNbll?ïýâkÅuë?%ºÇ² Â~?–UQ<f?¼ß©Íìi?%!'?¶nàЁ¨?ï›Ãá?ÑÎ"˜;?t¯[‹÷?'¼.å??~cï@–Ð?†¶m›×?ïn_Ӕ?€ñm"ׄ?'(RE¦_?y7ô¾˜?'?¸ÄÛ{a?pCÍ*Yâ?îçÿØÌH?‹È·C—'*?cl}lhd=?aY(‹rŽ
? I:ª¢ŠÂ?Š¶ÝG$t?ïþ¥véã«?¹Eºñç?\g±ã?)•ãÑ#Q??ˆ75?±Pb˜ÇŸ?ïڜírDý?qÅV›ùp?^;AK
h?WZõpbD?fEqç2…?mî¾.çX›?ï­Ó¸	­?q&Íè¸?vB·ôoFh?nñœØÅÖÈ?s2^£?W6­¦ç?ï·pösu?jb-Yòë?V…xÿ…k?B'[—åŒr?~¦&®·+Z?i?N21½AGN3FGL J1125.6-6012@rG[€#¦Î?ìû8ÀcïÀ9*]ÔÏÀ:²Qaòc_?î%%‹ç@ö%ÍD@ýÔ¿_{ç¿Ãîü'Ob¿æ̑'§†9¿èT–cjnÅ¿ä25w08,PSRpsr?äILL?Ç#ýÀà…f?µ…]wtì?³½™"?ÒŠ…ˆN?Æ¥Í]ÛU?·Ÿ©l	8o?»YÝÝÒj?¸Š»Öìq"?³ç¦•Õ?éú³W…Íà?Ã&ó´Ã¿?ãPIDUo?´©ãà™ñ?ºö'hhø?£¬Î¦Qôû?Ò¡äpb?³cÖà3ë?Ödù‡s…?¼.½W¹ÐF?·V:Ç)´T?®«Ôatã?â	)öÚ¤?¼bQ÷H?ë>¶Ù'ÐI?¾j,ú7?X\,k3?w8¸Ü"'?¾´2Vi?¼tj1)Ì?Ð>ªH*[?Í.ÌÂÌÿß?¹8¹]mê?«»øÞágÞ?乓°)0®?Îúð‡Î&?ꇈ¨Á[?©0ýµF1?­(ª^±èÐ?š33˜¬¦?½/e'\çÀ?¥†'üÏ=?àÞc$èl»?¶¹åCSK?¼'ãÚì†?¥
Й"!Ã?×Bo½8kh?´¦.X|¶MIXED3FGL J1125.8-0745@pÒäÿÉy[@H·&_æ¥À:oæÃ%À;ÎCG}m?'É£a>jf@ˆÚY¨=?ÿB*Z~&¿ç­¨,·÷†?ÒwF™¨™M¿äÉns{"¿ÙªaµEAGNbll?ïò<ÇËJ?Rf¤Ä®çÓ?AMq'*®?@…Ï''9?Rß·HƲ?M	Ç".
«?ï'ákaÅ9?‹f1"ý¹?yŸÛ¬:?yV§6™$?}p«*dÿE?…ñqº£?ïú+!8V?…UÇ´if'?†­¡*µõÁ?tè²jM·%?'ÉêI?€<këç?îèì"x?'$Y:SÄë?'Cï¾ËJ?‰¤S[2z?'チiþË?ˆ20•#\3?ïú818¡??kW‡Op?/™öŠžŠü?(«-''??ÙC.¸¿©?9Å»Ö\Ç?ïÚX	<¥ß?pÜ`Ʌy?aä%³µ¥ò?a094PS?cÃÐûÓM?fnšËqz»?ï'ã­—?tœ?G²Öà?|%ö»Þë?gyšC5Pn?7Áª°?meƒwï?ïÃçZž¿?m}Ι¡îO?lãŒ"q&?XÒ͙-¿}?o5öQ?f½õ[CÃAGN3FGL J1125.9+2007@l`xÜ@QO?Ï"èÀ:k™èsòÀ;÷úŠu9h?Þ[g/ö#@'ð=?Q@}?pÙ1¿yt]þkˆî¿ç	Ž8f¿Ûš+5Ÿy¿ïÿÎÍ&ÌAGNfsrq?ïÛr¸6ñ6?p>2м²?d®D(}g?fl›Æ,è?_¾™ð?bÛkƁ"ú?ìk"÷Š­?¹50ô2¥?³JÝï•ì¿?³ˆ(€mF×?¢¸³/0´?¢à–Çq?ìSÙo~Ç?¥Ô")ì%?±x§©a>³?žãße
?§Ñ vE–2?˜øEáŸï?ëdÚeÐÞ?±ŽÞ5Zæ?¸¢b%%Ç?®Bp>¶±ô?¨m•eʍ—?±>bÇÙ?ïñ9À¸c×?Y@5^¸pj?P¤Êì?PÛÈÄþ—ã?IÏâÀ!î:?IÊm"ÍrU?îìR©ú?¶4œú(#?–£9}¥X?–Gq¢'c0?‡™¸dBž?†‡¥j!Ï?í1oIõÿ?¢RöQ?ªbd
ƒ ?–­þÝ>°?™U
Ë!ã?K ÄoV?˜¦?!ß9;)?¡%X÷_iê?ˆ®Z	ëú?d®¶MbÁ?y¿…õÎ}AGN3FGL J1126.7-3834@qÔ_'`@5aTÿ5Õ¥À9üËE%¤À;µïXz?Ü{Fþþ3ˆ@ým"V_@)_ÊÀÙ¿¨Wx6ó\.¿ãü狃Æ
¿é¢<a@ró¿ÎìAÁ/N'AGNbcu?ï§áÊ'à?*ì3ÔË?ƒBi‹Ñ±@?¢LÈ9ýî?V)­5ù?UŽ€ò:èÝ?ïu€ûñ†?›'ÐÐêû?|é=Úú¸?'H}ïX`¿?"WÌTâÇi?•µ}'µ?îJ÷¾¤&L?•éí "?œJËóau·?Ž§ìÝRDà?šV<6aòÖ?†táâWÙ?íj³°¤«¤?¥ò0'ýš¶?'âéå#•?–rÌ2Ð?¯ãÃVhñ?¢õÀ°æŽ?ïíTFÁ^?lö[×»??]:ði{˜ù?k§솗±?@9}³Ý?>ZOáëäw?ïÃCwµ)~?"k¨	"æs?g|æߋSû?g=†h¥^?rŸÐª¦Öõ?€míA/Ó?ïH‡üî?'7ÐY|ѕ?ŠìÙ©÷W1?}˜G\O!?ƒDRã¥H?jÚ.k—"?ïQI&m?ƒw…>¹W?s;ÊE…ލ?l7užF?†F|…?†wŠœmAGN3FGL J1127.0-1857@qK…ߨq¤@Cʉ€Fâ=À7R_IÀ:æ3hXÔ?øbýPMJa@ð"gXSÔ@/8Ç¢¿àD¹¦h¿ä@W¡&«»¿åC¬':׿æ¥N…ÁlêAGNfsrq?ïõój'½?J4g¹–Dì?5&§?2XuKό?O4ݗ°Ôç?FËwÖH`'?ï¾ææ\–?€,uG‹u?l"­¸"½?pÿr]6W?r"BYh¿n?u€@Ã?ï--ó>?'];:*Ø£?Œ'°DÂ,?‰
·÷¥(ô?ˆ¼ÌÌb®?"&Ÿú _ù?ïÝÏy­ôx?|فÕÇa?7<•"t¡"?O,PŸ±­ ?oHó}ªi?|sâX'Ö'?ïùûñŸâU?@çq²Æ?1É>E@[?2ý&ž‡º~?>W6ÕW½?7*Uw¶6¼?ïç!'Ô¨?d+^µ?W‡L¼þlè?UF2‡CX(?Z6c°ÓÃÉ?Y¡ŠhtÀ?ïmíaunu?…á§^Û?ƒó/E;–?€fì8˜?~´ihIL?{ՁâýÀ}?ïùÈ~™'?PLÛ
'?#¼Ã÷Ü?"«Ž€žÎ?D¶y 4?O(¯a4à©AGN3FGL J1127.8+3618@f‹-ÿ'+¿@Qƒw`MÉÀ97¢ô§À;¢1¿•¬¥?å,>>v±@"¡Ì@Ë;\_¿Ùúö~ªˆˆ¿ç+Q í²¿åœšQÇÀ@¿ã3÷ã?Ä«AGNfsrq?ïüýZøãÆ?+ô™'Ïž?(Mà'ˆ0?"|î5ì$?'ÜnXV>? txPm?ïºØ©­k'?‡îþnék?n¥O`â':?'KutûBj?sAhZÖg?wqò8Ô¡D?ï?J~\?'!>¬¯â?ƒhdˆäÂA?u‡{y?ŒÄûУúy?x®î5—Wp?ï¾yÞú]?{K.Îä}?U?ç|s"‡?T5W®KÓ?{s D÷]?zi%Â'?ïúÄ
Ý?¦œßŽ¹H?ñ(ˆ6¥?°$c 9?AÑvÈ×3Ä?©Ôã¼9l?ïèÑS€kÜ?cIx5ó	S?Tí›>Tbz?RŽˆsHxr?Yo½»T"Þ?Z¹7_è4?ï¡2füÛ«?tú$Ö%?v7ë¶Wš?oïBX@9?y.à°´ß4?jf׸pš?ïôk²U¨(?W0<t'??§	|%ƒ?3M²wž1?N}²Q?'?UD]ƐbÛAGN3FGL J1128.0+5921@a§É`0Â@@K[€"ØÀ:hJÆͯKÀ;úÚa
¿é†ƒÛÓa"@
Õ´¿%D@¿¼w¯d¿æÜkûõ.¿æóý¤lA®¿ìzmôWß¿ïÿK'$°AGNfsrq?ïÉxáWE?€Œe=™V?d¦I?	_?pu3TánÈ?pðj›ˆ;ã?v'¤Õ(ì?>Â!g?­w'Øâ?šê½Ññʔ?¤æl©>?'":NêЗ?švMÙ	™?ì'«í%?¢²~-\£}?¯û­+Žýs?˜™RvðLY?­‰"l7?˜¶Ö°*Ÿ?ëí-L`Î?´yÑ(™Tº?´O±/l½?²oÞ¨X?¨È؅ïl? Þrò¨ãë?ïÞ¨+z#ª?xz•óžÕ?\¤&YÀÅ?doû*Ð-•?cWx.Õ ?p…#ÿV2?︉›
¦Ë?ƒ¾—$&T?r"]œë—?v}	Ñòõ?q'ÔВWC?sôƒZ ?íœU>S€?˜w—ƒm?¥6'ΩXÅ?'{ü£õ«"??Q¹+l?‹"ê­á¹¿?ïˆóœDnÅ?$f¶F4?wÉ;ä'Ú?v¯äœ'Áe?Þzüú×Â?xh&<Ò/AGN3FGL J1129.0+3705@f>A [À@Q~³Œ¼À:Rîº]À;ÁXù–Ys?Ö!¥Z@8É˳@¨Yÿа1¿æ^µÀ@ÍP¿ãp«ëº¿Ü(•kÈ·%¿åÌÔkÉôùAGNbll?ïþo6™š?"S9Ó?Äꘚ*ð?:à…#?$›WÕç7[? r*"ñÖ?ﮅ6é©°?ƒ1è.ðµ?qŗHF?tïçø'ù;?v÷Ícï·?{1Ñæ¿u¢?菉r/â
?q¶:‡ïí?p¸P0G… ?b.|G'̘?|èvÉ¥më?j<iDiŸ×?¤Ðë|?1i¯ÉL?ft`Ÿ†ÿG?bmU颍·?"¹~°Aù5?{qúJá´?ïÿQÓB˜è?Q('&›>ûoÝÀÒQ‰>óÃÂùõ".?
ÓG¿~ܺ?³'…e.?ïâÔÙ¼R?hû‹¦?Yní€Aõì?SÛª?`tƒhâbý?b'6¿BjE?ïÌ(áåQ˜?f§±'»?eÖ}Õ·º¾?báÔbĤ?n 0Y¢?W¼û?œ83?ïåÂ?]Á…?[۟)Ñ·¥?V«"4?EÓRÅñ Ÿ?]ÐjH˜ª?UÖ£ãdëAGN3FGL J1129.4-4215@qñÂà°«@2nÀ§û\À:ŠÉòý¹À;¿IÍ©kŸ?ޞÏà
Øl@U¸™9@ݵ_Ƚt¿ê<âcâÓt¿ÖAéV<Äú¿æ/–àÏ­¿ïÿìã~Ñ(AGNbcu?ê
'ÔS?Åßâڑl¶?źbÿvÇ?Å,š#á?'æ¸ô7Q?••ý'?êÏ*åܾ1?¹úÈÇy?¹¿2è,3?®j{Я?¯ŽëÐÿÿƒ?±gDI}nã?稇¤Z&?³FFòhùÐ?Åûìàh‹?®xÃJÂñØ?¶Ãé$Ê?§W3È£U,?èH¦d®*u?±gäÀ´e£?ÆÞ"WRÑ?°~¤CîL?¯ýUpqn? êï'?ê`jíoë±?Æ¢¼Çá?Ã\'ŸvË?Ä6¨ô~Ô?›¿½¶'›…?­ÉŠ­c?îMøªåá
?¡¶=;
Z?ž×^ŸhR´?"Xu??—iŒ"Z?šm¾#°—	?ê°ÅZ<·?­Vñ±ç ê?À•¶k§?¨¾ `ÃpJ?«ÎDhµ'?œ3óŸ	ö?íÝ%
f×?'»7;:«?©	ƒW%?|'8+‰~?'WKN.¢…?'‡¸xÄAGN3FGL J1129.9-1446@q3nÀrKw@EÕñŸêìsÀ8¤˜ÒÊ<ÐÀ;•¯,¨Õw?èãà:5@õ`ªåœR@Kà˜†Ÿ¿è.&Ãۃì¿èTB齿ìUÂõ]¨¿ïÿÆւqúAGNfsrq?ïü<4e¦?7A))V@e?/¸Õè‹	€?,ä°N6¾?,ƒäe—¡Ù?-¡›{£û?ï›!ÐÎþÅ?…""v¬6?wû@»'û?…1"
£ÿ?zsÖüM†W?ƒ'»¸{§®?îÙ¦óÛj±?Z1rëdO?"c2½2?…lø€ùb?±¾X´¯Ç?…
ŸËt΂?ïq…y"®Ù?b}=µÌ?€È~ð7Œ?†³™z-ü9?'Ö#šZ?†›üoL ?ïý‡`=‹?+SpXÍ^?(ì"1ÿ¹?%8s}gí?5Ðïõ??û×XÅC?ïÙ3\›-æ?o®Msù8?bR²XóQ?\eÚ)H¥?dyðބB5?gLôÂ5¢U?ï6;öG¼Ï?ƒ'â݌?Žaj©9R?}ªgó³YG?"—¹£Üà?vÎ#+$?ïæv9MÏ?mYæ…nð?Wâè»y?QA¤#"H?[ø«#
`?j\d.þ›&AGN3FGL J1131.1+5810@a¹/ßÁœ@Köõƒ¥À9üÅ0÷ÑÀ<¯k'ö¿Ù xA@@+­,ôU@EP¿`'³¿æÏÇ~f¿èkçÀÕ.¿ÎÅýtNJU¿çÎ^G^
AGNbll?ïõPM¨r?OôÜø^?=Ü8ƒ¾"'?8XW"4‰?KЯ7å9˜?IŒž+lÒ?ï€CEz?Œ'*áìI?€$Ȗš&V?ƒB"ðÔ?²Máã¥?€An]Igî?ï8ÚÅ?‰´Ç¥ú?…G¨óð f?sþ¿÷CôB?"•?_³¼?º~¬?ï?Àæzë?y~÷êS?p%æÏÆg?nä{»ò9?"þ…(3Õä?ŠÂANA?ïýˆÒ™?2?9Èf?#¹¦9?!•N®çت?*¦±wü^?)8¢~/³ß?ïÚÆÌé¹?jÜZÿíðæ?c6UvYñ‰?^#Õ>©;?b³ã»\}&?aa_	à‡t?ï›ÉoJ:·?où(Õ'ð?t¸¢úh?g—YO0ý"?}c2£ÅZ?aYjÇJŠ?ï݀g§;?d|
]ÞÈ?TþH†à¼?EʍŸ;Í<?ht?¨¡?a]OGÛÌAGN3FGL J1131.4+3819@eÄ_Js@Qv‹`òËÀ9Õô†O9úÀ;?)
»E?âð—	qmÖ@'þ'…@"@ "€¿è¦qYg-¿ê¬Ü-Ë¿á¢Ú- ¿ïÿÞ\
¿SAGNfsrq?ïÌì~‡´.?€>'#Ã?V¢V³3?Wil§%¿?sá+,xŽ?~"ºÐ¦4?í|pW<8&?¯hLF^ñî?ª"Ë៝?¨l›IGÈ?œ,^îýî?šjŒ]Ñ?írç?À?žàã×¢?¢çÒx ?!m¬äv£?¦É§°T?—²ièq±?èûìÆ£y(?³&—ö—¦™?¿ƒ³ÎÆ?°ïîÖ[³?¸z¼V)z?¤t¡Vk5r?ïí¢|0?oü²ÎA?BsF*k…Æ?=¾·DLq?[d`¸Í?n|š
ÿÌ¢?ï0$p«Aj?'"{ú+½?uëùêx?Œüèõ§€?"€÷͆¥?€jAӏ'³?î±ö¾sÿ½?ƒ$CHƒ?—"LÂ6¬ö?"'aC¼Ã??'žÛhj#j?…)?iwgë?íK©ûÖ>?–א:íe?®•8D–½.?"P¸ÖÕø
?™`Oø›½?"°U¢è°€AGN3FGL J1131.9-0503@pÒ: WŽ\@JC* dúVÀ9‡;±†ö)À;ž ùt̿햼CxÕ@'
L46@D)ÀmÃÓ¿æ
E")Š_¿ë/gzý;¿ë
r.¤?¶.w•@wAGNbcu?ïñ5)'…V?VBÁ&Ѥ?KdÉì¦?L\ìe—ðw?P	û¾Ê?M•Ej•?ïºsúC•?©DvðSè?o¤ÕQˍ©?sÈœM?r󘊲Ã?v0oY¸+Î?î_=½M
?"à!'•×'?"H?‹Z?‡mò¶f:? heß:µ?Œy™+Ýò?ï¡\16âH?"õ	hÕû?2Ëéx…±?@£!?‡›o#ý ?"ò¤Ý €I?ïùPÈøà?Z..Ì)&?5nЕ…Oª?3@¨¶u?>¨­
Úù?Y8ô֒±'?ïç$¾!Ž?jób¥?Wu'áÎ[?[Ax©³£?ZBF+Ÿt\?a-H™<³?ïMþŒï?…¡ñNXË?ƒÞ±)ñÕ?}ú5,³ð?‰tÂ»Ti?|îÎX€Þ?ïô`üˆëæ?Wš0ŸÝcô>ÿ	^âꇀ>þ×OPʶ?VÁá+¿y?WŠÒN:ydAGN3FGL J1132.7+0034@pƒõ_þmY@L´Ò_³Ä¾À8x
è³³À;9]¯Þ}?ãÛÏbíû@Æô÷ŽAw@™ _Æå¿Ýߨ¢J˜¿ã	¨ß'¿áÛ£'¬§¿ÝF‹(	AGNbll?ïöˆ‰•¯C?HípP7?@IØ¿àÝP?;IñC~p?E"¦ÜÙô??4ÙɆ–?ïiÊwÄ?"Ñtïn¢?'÷/†XV?‹*á-–‹ÿ?'–2‡íÄÇ?Šç)"»?ïYhÉd…?ê®$º W?ƒU?>†?yÝE14ÅÍ?"EÒÁ/??Œ|8 2?ëÀ»{¹_?«;qÒ›?žtBˆjç?–A 'ãö=?º]}šÌ?©Ï9D·m?ïúÎKì¬U?5ã	¸Á´?5ïñ‡Üø?-CÒ
€Á¡?3¯ÖÏ0?&dfñA¿•?ïÀl"#Q¥?'"¿+Ô6$?oº³Ÿ*\?z—G$™Í?oÙ)üü‰	?rx©u^ð´?àÝê›?x¹Ä
Ÿ(ï?qê»PRS?d·4ö\I?|ÏÔz©\
?tÂâ]@Ċ?îÏۀÕäŠ?‹OÑ©ŸXó?Š¤XA©‰?rêz59îo?˜²cÞÚh?ˆ€‡W€M AGN3FGL J1132.8+1015@opÛ ¸l@P=@GDÀ:gÍÀ;È©lut ¿÷EJ!ŒAÂ@
¶ža@ÃÉàhÚ¿èh ¼IX¿é…®w™‹ú¿éˆíñ¤ac¿ÃàJK0]žAGNfsrq?ïþ
ØÁÞÃ?(¥jé*©›?S8ö]l?¡ðÈ#@×?$Jù²5Ø?!-o_œ×?ï¾°£\¢)?‡±Tåú4(?mõ¥|²sQ?''Ú8hLÖ?q¬Ûš4ê?užË°‹¯;?ï=´0ý+˜?"cçEÿœ?'0?Cÿã?{R wˆÓ?Ž"Ê ?{¶¡o*u?ïè–ô<—$?eÙ?Rl?ìFGÕÌ?ÉÚ1œd?g
Zkd\¶?eÐsW1"?ïþÖH1Ù'?«p<Ô?ÒÖñXL­?'˜`¦Ú?M"Ý—?*ò×ÝÐ?ïè¶J²ßC?fþ
ïzId?Tkëw'?S¡w‡i¡õ?Z(RIû?`–4{"ö?ï¡à)öÉu?y"'ã)?séGï*Ò?pù‹JI?{&£â®šŒ?r'ºŽí}?ïüèôÔ0w?:– Þ×>׶dðôö¦>Ö"$õ<=?8Y€‡?:{ÆÝ©h.AGN3FGL J1135.2-6054@r\åà.©a?ã@?éØÀ7ÅÒtwÀ:°½L&I@‰uҕ
Ä@²,ðÎߢ@ÆÄuw¿ÝxdVRg¿ããõå8Ã/¿åêybru¿ï
$p:PSRPSR?Qò¿]	à?RmqÙõFï?îŸâ3™èý?©®£?Um?¥rFÑBÖ?©sˆ.r¼?7lyÌ6?SuÔÝÛDŒ?éÞeGú¸?ºJt>&'w?ËÐÐ+jÖ§?º@¢ûuµA?«€úzB.?ŸÐ5b…?éÂç•>ÚË?±''Ò¸o?Â#¯
‰?¬¢íµ†Š?"<Õ>zô?x~
EÓ?ì2¿'6.÷?£Øá¡"Ø{?»âhÍ@\‰?¢FcIxy?OÁZ.*?S•Yzd?ï=Ÿ?BX?£Ÿ˜WÂb$?žÛ^ú?£sx¿ü§'?U/Ӌ7–?l(^X¦æX?éÐ:'»²?°—ÇoÉD5?Ȕ¶ì³ê?°c3šÐë?»;–2u·×?¥œRÚ¹´?é~§áèà?­Nâìé€?¸Ï1"Ã3+?¢š*W$P®?'-›¬‰Úa?|­
«Òƪ?ì¡E\LÿZ?š4V%5 ?¶jn3¿i?–&€ÊPSR3FGL J1136.1-7411@rœn «†À(+Ö@éÕÀ97oJ:¶µÀ;vReþaš?é"ú|C®'@
{JÍǟ@Þø 7­ì¿äÊ<'zÿäi˜¦ï1j¿çNµýƝ¿ïÿ¦CK.RAGNbcu?á
œÓ&{?Éû•Ëapf?чv?çˆ?ÅÑÁWèc?ÈÆ£åG?ÀÌz""†?¹›ý5Æ?»ã'&¯J?å#5˜×ì?ÄÀÝD-Y?Ϊ۞ªX6?ÁµÀŸJ'?ä¡çÆÎ0?±'èGat?ÎH%"brç?®.n°ëM?Á•RϨÖ?¢ÁåQεÍ?Ëú•Û§Ž­?²m'Ü`b?âY‰³"äË?½xÓpÙÿ?ʟCX*Ÿ¢?²#×¹yƒ±?é(ìÖ¶
K?ÃæNoQœ?À.ê•êù?½€¹4$Ûé?¶ZÄañ¶?³¸n%Ío	?иUÔ?TK?ÃiûžhØ©?á'´·›ý?Â]"þµ…¼?ÊM
†È¨ó?º}OGL+
?éÐá·ôK?ªP(H‰áµ?À?x!5?¤ºõðî¦M?°zÁÄqc¹?–`E
?àw/nO
w?±‡5	?Ö^òùÿ'?³wìñf|?Ág(`Ï×!?¤u!WM MIXED3FGL J1136.1+7523@`#W`9%»@Diœ@=òÀ:Žã]2À<*rÉK8¿Ô}聴 @ßF&ñ}@h³ UöW¿ì5=Œ«¿Ü£CÑ9Þ¿µ¥úw™®¿ïÿeiûØPSRPSR?ï<
¿K°?¢®ðÏó?•;ÝIôJ'?¢&•Lÿ?jOÎÕ?mo¦3a}ˆ?îH'-tàÛ?¬7šD³í?žÍô°¬?¢2¬þ(Ï?˜!Å Ô8‹?›Ð4€T?ë.5ÞfÛµ?¦ÉmEO?¶‹¢Œ?  ÑHìà?°yÅúnÈ??rÁ¡G#Z?îþJ_ìñþ?™Â9ÌÝò?ƒo† ð‡[?²Þ7u?–~ð¬î
¤?'©y—Ô?ïfÏì"8Ë?¤GŠ5×?rßaIÓ?£îF€>?eŸÍYN?e=' @IÂ?/\†`?ŒÞIAæb?'NÃóºk?g‰w¦[?|ŒÊÇ«?~Y+" ?ì'IàW?¢\I>þ¼‹?²8	ykõÉ?•´'Š%·?¢kO	v¢ÿ?'oY|)?ïÀT֓l{?r¾Ÿ×Oi?oáHïWó#?f/:ƒF4"?oÉà¸TÙ@?häˁS=ÉAGN3FGL J1136.4+3405@g‹y¢ƒ@R`×óÀ9ß]ÂSÀ;åðL-Õü¿òƒÐ&žzT@½e{C@ ¢àRG¿çƒvãÈM¿ìWDû»*l¿ßýx=uα¿çQB,Ë:&AGNfsrq?ïú²~ w?Gš–ýŸüA?böÄȜC?ƒ9E
'?B)§}	Ñr?Fg"œÞ·?ï¶[ƒ€Êã?‡¤õ¼[ðª?päñŒïÄù?'~C>Nˆd?síL«¥?u³ÆÙ´?ïš©+½?‡P…Äô'ï?z–,ø¿˜?j´£\ÒC"?–g¥µý@?…ç}Û\Ž?ï¦	žÈ? }3<"t?Iáýˤà?Fºý{1;?"ßx¹щ?€ˆ¯pV‡?ïýZíÚ¨?5½ß¸DÊ?HA;¢:?³†²å'?0]íÓKü·?2Ì@""?ïäLË=?g'Tf³?YZâÿ/?X<nGg¼â?^‡§Š§?]6‰DÞ?ïæ'U…C?}¨î²¸ì÷?m¾aÌ)`?aâx˜à'œ?"–ÝÏÿ?|§¬_œ?ïó×ýqI2?U«n©¼?!jBàÆÐ?µRƒ¾oë?V"Áw¹\ô?Tú۞6åAGN3FGL J1136.6+7009@`|ŸŒ¨@Fӂ PˆÀ8Û°hjÀ;^R_Hdô¿íxGøI)@²ĆW?ý-;·¿ÓFãh3‰ß¿ßºˆÔ©¿Ü";
dS¿Í¥+OO7AGNbll?ïoÚNÑ°s?'΀8ñú?vqßͤÈÖ?sÞ¤o&½?ˆÐ|d'ô?Œ Ó´Bs_?鶴8'?…'0+Òþ?räüÿҁ?qqf6?é?y,€!/ž?q¾ÊÝ´©?íÍÓ#^#?™ª±iÐñM?›€í\×u?o©½û?¥b¾×Ë?'hÈË&?î?Rrµ÷?›ëè	Øà›?Xs€^
ë?_æԁí@Ž?§Hnڃb®?›£zc¶mA?ïÐòýÈr?uù×Q÷ø¬?^Ñ!ЀP?\¿ã"®9'?o¤x¶ó66?qHQ¿¬?ïߕc¡\~?køà$c#Ë?]Âã8áZ?[±†Ï­Fß?a‰*¸ô©d?dGúvCu@?îðr$Eë®?â£÷âg?%ÚÛ-?'ŲêŠ
M?'_3tÕ°?"sîbìWÛ?ï¨É0qH(?yÙ*©ôé?5_ħÐ߇?-YøúxÎM?…"µ·‡kD?y²{µ$†êAGN3FGL J1136.6+6736@`®.oKè@GûrÀü¨À9À®9À;"Í.œ?Òוù&@gғ`DŽ?ûe?õ¹U¿ço@Aä{ë¿Öà0^l¿Ó—öÞx5¿ØF€i"AGNbll?ïùí¦ÙjŒ?:Kg#°Õ?7ôýv×)?0w`â¾?8Ì2ðò?.8³›e†?}?‹Oãíû›—?x‡&̆ϒ?v󑼑Ox?€
¥6I	?†×Û¬¡z?ïcA$Q\Ù?~³4¦tü0?€:0ßc*Ü?sGxó…k?†õ†L@å?rßú¼H??îÌ1ž[ÿ?)Ù~r2?u.ô™¡O'?s̋sc"? —€ÀT¥?Œz9í…ï?ïüۜ.°~?+m1\¸èÛ?+ÖÆcç²?#ì‰æºÅ"?&os$ÞÎ?ÚyW2­"?ïÛÈBùù?jZ¿ç¨š?`†25f§?W¢"ß
ü?c±‹›¸7?dì0Ýþ?陋¨š¤˜?t Yx
?v™.v DR?rA<0íé"?vý)‹ì?X¿—ck*¸?ﮉ'l£º?nîêq|0?iŒmt;!?V&
"=é2?{õOaÁ?i÷áTl‰ƒAGN3FGL J1136.6-6826@r'?…Q
À=™àvpÀ9"Í]"ÍÀ;$É3»o¿ÑW R°Ñï@0˜ZT_S@¯nàˆkt¿çRšNÛ±¿ë>5oÎo¿â™þƒÔ
"¿ç4!ßñBAGNbcu?ìÌí¿q3?·ƒw²•É=?mE{ãçͯ?jüb¡ڎ?¸®kúÚ97?·TVò¿ u?çµÄ@ôÝ?Íè"ÁÎʆ?©Ÿ!Ž?ªUö "…o?ÊãG7¢Ê?ÉĦbªÅ?ê¬`Eºõ4?¨±%;ù«R?§CA"jïs?'m}güìå?¾û]òÞ§?¥vHPŽ©J?è;á\s?à?°Çž¥.µ?$">Rúc?ƒ¢O°ÍSå?Íè$°Ó6?°wߝèfd?îÚ¥
™"š?°"Á×…p?_싴̡i?X9c¢ì?¡VJö"']?°
ÏcýkÖ?í¤€/Ë?³soøDX?'"LãzK?–Þô½b¾À?¬nV›~\c?®
Í
`?î0]–f¼Ö?"Á¯&7'?"Cø…ëÅ?ƒ^ÚÒL?¢òš½‡À?on€nØÙ?íQˆš‡š?•o°ô?±–>³?h¿Id?³zÀÏɈ?" ,.&ñìAGN3FGL J1136.9+2551@j¡Ì Õbž@RS&@©À:e¾BÆN.À;¿þraFl?âeë^¤j@}þraF?úÝ[ d¹é¿ëœn<7''?Â_âfšœW¿ëD"†âÝ°?á|«¨‡@AGNbll?ïãŠfÔS?iÿÕ« .Ã?eŒ¤?g}"S£ùi?MÂý÷ —?H5¿uJ
^?ï»jFÅ·/?D?H`/?lùïÊT'?t7˜ñ²€?sÎR*²N?ua¥»?îˆvþ"?—¤‰ˆû™?›Õ ¥´Qx?"BŸ¶‰?"*p'Ä€Q?ÐÅ=Ê?ïœlSªø?Š¦NÔfƒŸ?oš?'•Ãø·m?%a"ä¾?ƒ·3ö¹¬?ïö«Óôg?Rþ»÷°WÏ?EpLÁ"Ö?NåٖB*??†IC.³?;t+%*ê?ïç°:<^M?fñGǒÞ?VlÍ0ƒƒ?]#Ú.ÅõG?Z2¾ÍgrÇ?Z»ê@>ù)?ï6á%tXÂ?‰	³¦î¾P?î‰ø÷)?…ãŽ4œ??"Y,´AzD?r¡re'?ïòÄ=åœZ?\º}qÊ7'?B'fÕªŸ"?K`æÍvö?Q6PÔð»÷?Vð¸ÿ®SAGN3FGL J1138.2+4905@bÙ`Ëò²@OðÓ?­"ùÀ:U:ûÀ<Êý¿³àÀYI&‹Ï@1#õ'´Ð@Í̀{æU¿êÿè¿âxnùÝÒ¿ëèé¸ëÄ_¿ïþÒ
ØkAGNbcu?˜§ù{?e
å÷*?†…#öZ??Œ¬Ÿ,kóã?I]†žìÿ?PÉm¦?ï¿rÿy?‡EÃKûž?k»ý' Àì?'D.—½ØZ?r'Çä¡Òé?uÒ7$ñZX?ìӄ!•Ú{?¢gÉÓH<?¯ZÙù?šgA—Iê!?£m âöS?"¶aŽUçÀ?ïæðpA©?q€êõ¤€×?1Ón–"C?M‡ҒXt?fîr;D
?q
Ê$p1Ÿ?ïÁ*@µ»?¹H£î?|ËËüˆs?Se|4o¥?FhŸ®D©À?EAÓqCž?ïçE` @?gKjQÏuà?TÏá"]Õñ?Sq¹‹fwò?\¥^o\9S?`4T)ÿ¬?î
µJO/?–Õ×lËË¿?¤IÙæ+f¸?'Û`ÈɆ<?"
•Îè¹?‡ÙØЛvY?ïüO,»1?O%ÔC†Ë>È'éÄK>óك«¹N?=VMjh`(?O8Ë>êAGN3FGL J1140.4+1529@nM߆ã´@QtUàeuÀ:¤ü4µêÀ;£ÀÌäJÀ
/0ÁƒÃ@	&z?É?ô $ sRˆ¿ïÿè¤Þ`?ï䉗mðH?ÓùÊÁÚ«]?™õ÷­9ù:AGNbll?ïñÎ6YXa?^ÌO–™ž?3ö/ZUGð?8úÝs'ù2?Wfê,ˏ?[‡[ý?ïµÇmùhó?žU·že¦æ?hοڍ¸	?nì¾?x´éÆÚt?¦çóµ=?î7ºÅ`ƒ?›®ÍsÀàé?žü]¹´?–vÐR#Ÿ~?š dsxò?¥ÓoÆdè?ïñ0"ÃÛ?d=ÏöÐ9ê>Ï"]a±!/>㧸Ð?]9rä5a?d7"ÝðP(?ïë­Ã…?e®~‹ôZ?3G¦IÔ?7ÝfU	±f?bƒ]v_y)?d³°ªÚð?ïè¤hCz?jÃÂT©E£?T¬™øK?USõ:í?Z(OÆç?e÷g¨¢Ji?íåˆ!	Ò?¢ˆ«N'¢C?¥Àb Ó—?žÄ3?*^å?—Î6ž‹?'Þ×GlS¥?ïýPOp"?4
<J-R£>£bô–)rÖ>«-
/yà$?5sÒØ·›°?4ËR
'ýAGN3FGL J1141.2+6805@`'na«@GÙw·À:%¾<çÀ;ò… ¾Q	?ç`jŠ¶Û@°:6?ùÇ:aOÑ$¿ï÷«z9#…?ïþ9tüèZ¿Å2×BÇ{¿Ëå¢oÔîAGNbcu?ïúüX‰6©?=dö&z¬?-º¢€N¹T?'KÈ8vÙ?9?è©qZæ?7\öË?ï'0Øÿ¤Õ?ŠÐ'Ïâ7?yóº†&Ù?{1œEøˆ?|óØä
²?'âéyÂÂê?ï<<2zˆ?†dIŸ"?s]7Æ_?s6(ύ·…?}–,€¤?'1À2Þ6?ïg™Õ9á?¿9 ¼vß?‡ÌæÇ š½?ˆÝÑS?|™®è5^?€{ÌÖ
7~?ïü}=‡8Þ?3/¹yÞfF?"›='ßØd?Ùe]ßEÏ?2ÈuzÚ{?-ݶ,?ïÜjÓÍ5í?n¥îè­??`p:u}ͺ?Y™Ë?ôT®?c$ñx"•?g›eؔ/?cåéº?€òWKB÷?v±=ê2?ijE+uÕ?ƒ9È
Êc?PìQDÛ?ï̫ο/?o]j©–?tõÂÄF$¬?kö*vC¦º?RÑW
ÔËn?P|¹hŠAGN3FGL J1141.6-1406@qg¡Ո]@Fµ| À9ô¤	_$SÀ;¿WÜ_çÇ¿àǬø@&Fæ™R@gãà¢J¿äþøÖ7|¿ç†?
 Á¿Ö¢uµ'®_¿âêM{³Õ…AGNbcu?ïËL	©?x`%YSÌç??pœãä‹?;ÿÚK&R?xbñ'ƒ­?w–Hô?Þ!?^þËÊÊ?|s+dh?"Yo•µm?(sn9'?ƒ"|òþ?MÏ0?ì©›v;ç?ˆHBu+·?tªÖÃqµt?œfY›ê¼(?‰= Ø#ÙS?îëD²•¹?‹ûo€&?fü6r?blÎfàâ?ŸÔj%ÔÐ?Š}"Å
T–?ïñÝѾ	w?\W$Äàþ?-Ž®ØµüX?*ò?£¯ù?X'†?Hº	?Z%ÂÝ@&?ïÝMç6ö?lùÝÇî©?^èÖôfl?Wwÿ¯dê?c=­~3§Ä?g=m='ö?Yj¡×?uœïß&c½?vy#rïã]?b,¢aʎo?ƒ×ðW˜?pª;]°?ïÇ3ӗ]?hoóé«Z?QYÁëù"??³ècüà®?x¥Ú°"C?f¿ä ۀAGN3FGL J1142.0+1546@n'¨`ܹª@Q"ßÔŽÀ9ßÞèXÀ;´¥hõX¿ÿx9ܾ@2Qç3Ö@^È •¡½¿ß}3£VÂì¿ä€Óð,£L¿äãތ<å¿Ú1מ7
2AGNbll?ïìᔧcÔ?WEÒAÑÍ?M©¥d½?D
"†np?W¼Oê'Â?Rni9?ïÅ»¤±?|Hz"ãÏ}?hA»ÒJ°h?j‹ô!Ý?qRD\ܒþ?s"Ø€Zf?-??'Drú=m?ëSÂ]?¸–¼àë?šmèH¥Í?‹®#k_?ï¼w¯[o4?|J'ÙÊJ?$¼VY·z?/ARý5?€'¡/<'?|rìü)+?ïù¥;–ã??Ç८è?:菫A£?2­•¡%Î?<bÃˁ7Ó?5=ñÁ³À5?ïç~­Ɩ?dàùê¼Ô?VFb¿?Vm,<0ù?ZÑ_Ñõ?Z ="!tc?ï|(7µ+¤?VxÏuü¸?|'Bzµf?pò*öìå?'ò(öŸ&G?u2½Û'?ïõïÍF´?O
ú*ZFõ>í'Ë×qè>îcæmY?Så_éë-Å?NûháÖÍ>AGN3FGL J1142.9+0120@p¹7ß (@M·ç 5)­À9Ì·áƒ=7À;Õ§uû.à?ö!sЇA}@
«¼±Ì–?÷Y©™èt¿Ù™‹Ð5ë}¿ÎðCgó7¿ÜN×+܎¿êÎd~§[PSRPSR?ëó)³¶.?ÀeܳŸª?·ñ¬ÊÆ/?¹hxÛÑ%? ëaiOÅ}?­Á@B3'ï?ëçVÂ?¼??¼ä¾Iëö"?µÅXëû{?¶Û³€"?¥ÿãÐtw ?¦Å±óª¤?ägóÙA$?·ª®ùÁç/?ÐôßÙwˆ«?´™òn—ÄJ?¸ìèéà±?¥Jת zt?éuèiWÔË?´¬Àí	r?Ä®‡˜ÌPa?³0»D¨ë?¥ç[™£Ô?œH¾K.ñh?ìxâ­â'?ÈZè?µQ1÷¤å?O3níI?›žâw¼¡?´õØá-?îq«Öux?ªª}÷î? ÷ùˆœ"?¥¯õ6ßvY?µ%ýoËÎ?›=7âÓ?éJ•,?°c^¶¼¬?ÃA‡ãþ[?«š¼à>ÆD?®P¨rðû? … ‰êþP?썒Åjü? ‰¸{1?¸æÖ.z…»?ž óÏ??…d.;·?:e^+ýAGN3FGL J1143.0+6123@a® ý;*@Jïä ()À9`¸K5ˆxÀ;ºÜ8zšÑ?ìX€ŒNϾ@}ö۔í@+¯ >ŽÜ¿àFc'²°Ó¿Þ¨ÑM˜˜¿Þ	©æ²•Ù¿ç?+õsAGNbll?ï1þ7Š?'nò5˜çc?‰Ù0ÂÇc¢?†1s‰rW?‰§O*¹á?ƒäEûéñ"?éHwºÄ?Â-NÛý¨?ÃS}ÃÀr?½Û‹­6ž?®*D½z?«ž!ýK‡Í?í¡ìÌ
ì?Ÿ[ÜÏÃ/?£ê¬la?"±g͋çê?¢SI?ngØ?Å
9>O?æ2:‡»JÄ?³æ•ÙÛ#?˝hÜ…Ê?².cS,»?·3Z
z'È?¥¸"%~m-?ï¶Ø<J;Á?vÊR×c?q·¦¡G>?h‰˜ÂɆ¤?rÜ;2»©?l&,~©úH?íÐa j){?­ÎC&gÀ%?©Õ'L:º?©Ü+J­?"´!C#??ÃÓÂL?ï)¼©Ó?'¡ôT?';jÉ»€?";皀	Ö?>¼À"8?|
8Sà¨#?ëûw6ºž™?œdòRURç?ºuöo;*?–\úƒž˜w?–¼½Nï@.?‰}«;'hAGN3FGL J1145.1+1935@myA HàD@RBî?äžÀ:Š"#8mÀ;õÙ&wc?®ÒDHî×@
ĎH­˜Õ?ÿ¡7€ô7¿í+ÈÐé¼ó?Äé3ÍY\	¿è±Ëi W¤¿ƒõ­…x"AGNrdg?ïÝÙ/í¿?l_–÷Ôf?^ªБ(å?aOÿÓO•?bÑÍw—
?aX•GñJv?ï¤n–5·?Š«Tdس?u	.^°?€áxÀÃ?x隺ã4¨?|9á){{ƒ?în‡!œÝÇ?"8´4Ú»?"ý…VŠ‰?…@9'ªC)?ž1–w'Œ#?‹üös)ç\?ï\2/ýô?'J†XkžV?'"¢"ðëô?‹{RÁìö?†_ÑÑãDÛ?…RÕ:±æ?ïôÕÚg•?TèÞeýf?Ckh–©T?FºÂ½¹_?L9?9[Ƶ?J€(ˊø?ïãl݊‡?hhí·X:?[•y["Ô?`~oL¨ ?]Ë8Pë?ZtӜ´©?ïM2jáJ]?€÷Œ*Ӎ»?…;ô ó¢?u[þ‡E¶C?‡xQAÞi$?tÜßMÁ>?ïèYgNU?b_
û2?T‡Gœ?QSñ}[ ?ZÆ#Ãݦ?Z{	AGN3FGL J1145.8+4425@c}ËßÒc@Q[ÖÀÀ:ß­FÈBÀ<B‹•ÊØ¿§j9DZ`ß@"óM¿üZ?ýšRaKÊY?愈bBH¿Õc8ÉöÑ¿ä:kc{O'¿Ê…û¨¾‹ÓAGNfsrq?ï걗<G.?_V´·Ài?Rd"°úÔà?TŽpñ"½?X8<ä5>é?TŸH–Û?óEîˆ?i[ŠÖ_?zBYÙr
?ˆ»Ø¼LÕy?z|¬u'Ã?€~úÍO–?îˆÃ
†P?'/ù™«ì?"¸ó'íPh?…ŸJN%ÿx?›FTaå‹?‡á¬K۝6?vÎ? ?žø€2?VȄUÊ?"HÙåCy?žR¶»{\;?™ŽãèZ7}?ïö(­Àt?WEퟩÎ?A²X­@?‹?Sã‹Eò?Eªðžì]?B0!"?ïÜ2åL?n}•t0'?`Q`Â?b²2ÍG?cÇëûZ?dhVS'Yú?ï?]¸íÇÄ?ƒ—â—´Ç?‡O'³ñ³?}x{ê±í?ˆÙj«I¹??wî"
ä{?ïÁÎæqRl?v‰‹RÅL?g*ë´3?^ÿÏ`a?sƒˆ3‹_Õ?s8ï?ÕaSAGN3FGL J1146.8+3958@dŸÙÀe¶=@QÝ­À,«ZÀ7ê$gMÀ;[(fP–ñ?î'l ö«Õ@óN¸IÝð@çÀC&›¿âdTÆßV¿å14œPz¿å^›ÎÔ¿ç蔘AÅAGNfsrq?ïû³âðû€?8´R¾"er?3QÿŠIŒ!?3æߐX6?.ÔUz?#¢ å3Å?ï¾ e´Ì?‡4‹ú~ô˜?mse}eå?'jÂ6]ï{?qöuÙ7?uåòÉÇÅã?ï/p04a?‹˜7JÃ=o?ˆã›q"h?ƒÆŠ@á?‹@XԐ71?ƒ˜Û³¹c5?ïñœìÏŒ?d{7¼Ù\w?&IŒì°'?=fŸ2Ò£?Yüõ(Ÿ}'?cë2OrØß?ïý²ì¸
Ú?)ü—)BâÕ?'­URê}Õ?%T$¶Èÿ?GÃû^îz?ŸÝÞc??ïèv3cÛ?eNúâ{_?Tø‰"¯Ö"?UÞV8!)?Z\¢`?[
ê݋ŽM?ïbìLÖ?‰•Ñ©y??…9Ï^?"zKzn²n?'B"f,ú?q*BQfÙ?ïýÝ µŠÄ?>RJà™?àðà¥Ë‰?"áU´ú?+õ´2c³?=oÄa:iAGN3FGL J1147.0-3811@rß 'á@6ø;‡}À8¦ìAÝ"À;l©èœ6,?ê4G;9"G@no+¢@îàrñå¿á¨g€þÔB¿ä¦÷»oÉ¿â®
Á"Žd¿æBDý¤Ê¿AGNfsrq?ïúÅQ"ƒk?:¶k
gS?5Î_nÿ£?2lY~ÉoP?4
"Ôœ?-ÔMûG
N?ïkÉÕK¡i?–¯x
û?}˜SÙ#ýË?ƒ^ìåë¢?†A`¸ö'Þ?'p}–ƒºŠ?ïA±ôC?†…‹Õ¾?…Á"Ve>?'ˆb)ŠÑÌ?‰öú€‹Áð?u¾ˆ-¹á?îšÞ§"' ?š@M'QÄè?'Þ°€5!y?x¼dUŒ?¡šif4¸%?™ oÔQ»?ïýpœRå?/n‡UÃ"ò?)s¦­î?*‹1ô%mÑ?IZÅ°Å?™e‰.¿y?ïÃ"Îzæ•?~lÇXŸ ?iÚû†­?`e®ðÙ?q	üò?y‡ûÖuØ?ï›4¥_[Á?|†`û&,?z\'/И­?z¯Á/Up?x	?n|?dú—äcq?ï£N_o¸[?yX'¶Ë?r âàHÎP?\´¤£=%]?{·í}(˜"?uÃá4èAGN3FGL J1147.8-0725@qJJ '§@JÇÀ'áÀ8ÊoÖQ°ÍÀ;g9
É<?Üú(t,;Œ@íËA\k¼@‰V  žñ¿ÛÏ|i¿åå»ëpk¿ä®<ì%¿ä(ï¸_,‹AGNfsrq?ïüTX‹¡"?1og›ìI8?0ÈsÜy»?+ .æʳ?))‹ÉΌL?!kƒÜ5ß?ï´@ìÚ3h?‰©–råÔ?q[Á® æº?ƒØ¤Ž˜žB?tƒÇßuñr?yin̤?ïC´'±\ž?'=Ý?"HšGoMf?y-Qºb]?ŠÊA\_µ?tT‰üÖå?ï›YC¬ìÌ?"SÏoòˆ?Våÿ™c?VëGÒò?†gU9»?ƒ–*¨ºé´?ïþ1êïÞ±?"È;ÀQV?"™tÝ«¬?è°d£Ç'?o#Vö?170:£?ïæËØtåt?hz'í?V•TMþ?SâÁüO¼?[Òú柚?bUñ'îžs?ï >|(?x¥U"êæ;?w_¤Lf?v8ÿdG|ê?xMT=
J?cüsœ=Ô?ïí¥<þ:?_K¦jº??#(tØ<Ê?2tAçõ&?\ì¼?¯˜?]®é'{âAGN3FGL J1149.5+2443@khÌ Õbž@Rø. &{•À:SYäwä=À;êúµ=d¿ù"øzût@RK»jNÓ@ã"@>^Š¿éI \ŽBÆ¿ÔmPëªÞe¿ç%+~ðI¿à±60"›©AGNbll?ïöj 1ä)?LùP1À•s?<õëÇ???qÑú½?Gډº
}'?DM¹mà³S?ï¥;ÖÅÉù?"OÜ"²?l"Ú?α?r76f.3J?§šÅßå?'ú4½è?îýÝOô+ƒ?‡ºã4PO?%ßµ2à?€5¡I~µ¦?'±f!Č<?{Ê)lP"T?ïˆÍ•/ã¯?"µÓÿ˜A?K)tÑ+?QÀې֚¶?Œ~"š?"0±nœ?ïûž*'½Ç?5;â'Á´?-2aô\Ý?)Aùò¨¢'?4uzCh?+Ϭ¹ÉÀl?ïäp-Bð?m#mC(Œz?V/™:™?T™ñýä"æ?`:ߦ£€?föþ3(Î?ïz–êÆ:•?xám©âÎ'?JȞ:xW?tI×Ç?€|º-ÀZ?cÕPؑ¬?ïèûK\Â?YüЙ_¶?ðð\??!R	F#S?f-4Û,D?X¾£Ç|ãAGN3FGL J1150.3+2417@k¥Ë èBt@Rþ)¿ìêzÀ8ÛðòFÀ;Q†Xt5\?½×ë4¨Ž@"úõT*z@³&ÿô"¿áظÀrù¿ã•Lo:P¿ÞyLOÂh£¿è•ñÐ"¨ÞAGNbll?ï×)–‡?p¶·IF\¾?chÜlä?gU À‡H¤?eámY#ü—?dƒ8¡_ I?îÎÿ…Ö?£G±Yÿ¥½?ë¢li­?'ºÐG–ò"?•4}ØÓI?žoJüØ¢&?î¡­Æœé?—	"‡:{º?'
G¬¶»?ŒÊ#V²Ç?™¼ÿ—}Ê+?ÀúTÇ?ì—.I-_?¥·H;‰?£—"\£þ?"hPTôN?µ¿|Ý­7	?¢ÊxC '?ïß7sá%?‰/8ø{©?hNÁû«¼?ˆå÷öY(´?P󕋲n.?YTjŒý??¼9ñW?$=íŽs?z¸æv!0†?¾Táo h?};XH{ý?ƒÜz¶Ì?ïn2žÉëW?ˆ …Gy?~ìZÆôëU?{ç%¥gì?"ý*áˤ"?O<¹N׳?îðe['m?†8°ùòÄ?ŠžÍW?tÚ:§Ódˆ?"¤LWˆ8?'·ç̽;AGN3FGL J1150.5+4155@cã{¼¾b@QªÍßòCÀ8P,‰ËÆ=À:î"Z•wÌ?èÚÈ¿™U@Ü"¡À…?ü$PôF¹¿Ñ¦àvo?u¿Û©S1¿Ù
ª©ój,¿Ê=.‰«:AGNbll?ï¡KXì?…
õtD8?keø"‹HÚ?ib‰ú¢˜{?€åo[ÂÑ?ƒ^Œ`Ì¢ž?ïI<u\?Ÿ†½ÕÖ9G?…÷QȯÇ?•	hR‡ˆá?‡¹ÐŠV?"àU:¦p?ì鬠É1?¤VÂfcّ?›lØöoÁ+?öRaÔ?±×dÂï ¯?¡X
5ÁŒ?ç6ä@ÿs?´5ÚKO?¨Ÿ2jp¢?§ZžbA?Ìü¢c¨Ø?³ikBƒÐ?ïÉpޏm?zjÈÆæØ^?Y‡O'¬?VYÆë˜\0?u†¢ÐÍ?xÔi¤3{ƒ?ï¦S]ÂuR?"î!5xÀƒ?yeÎ阰?æìIŒ?sp'3|#?{ÆÜégœ£?îxöÆgÐ@?–müÂ9Ê?†·²(Ÿ?…8
z? -8Þd³?'¸}m:¬S?ìe˜Ô³Ý#?ž%U‡½F? Š¹Êȁ?Y­ìä?´Ü×Cäª?š'2BõAGN3FGL J1151.4-1346@q—¢ŸœèÙ@GIZ _†xÀ:(8_ÂÞ7À;¿?']<¿Õ-Âvî°@éi{Ð?ÿ«@àoí¿ÜZ§žó~¿çÁ Hõ½1¿‰s¯,Ü`¿Ýpà~‡½AGNbll?ïýŸ£º?0""éhH¶?…ÖñîòD?Žn•Ì?29"8Wµ?-췂Û4?ï±	wÍìÝ?€Ö9?4Eô?q˜‡Øm?p;À
÷žÀ?uâ¼>ß_´?y4ˆA[UÃ?ïZ¦—X÷"?|5ëÖôŠ(?{gôŠÈǸ?füé E¿Û?‹¢_å
£f?uÌ#9~›?ï€&{¿¿?"ÔY£%Z?@~êœ|ú?EW®ÒŸ-?Žß|ûzË?ƒÅ­()°L?ïþO\šÆÑ? èèÀv?Ēc	ßb?Tsï:"?#Y'Œ¯?F"0+Ë£?ïãqjŒ¡ö?ezƒ]#èÚ?Y–h ͘`?UaaÜ´?_†ÃLŸ+±?]–F¾)?綾íO¬Ä?j?æÑ®ÿt?q‹—_f?XL6ýww?{¤~/söž?c~$4õûy?ïè÷ªŠÇ?Xæ'nøžF?7š1/æœÆ?-KírP
s?eÂY†Ð?WI¾IÛ AGN3FGL J1151.4+5858@a(¿;ê'@L>­¿ÁKÀ9iëBÙÏÀ;¥ÒÐçÝ.»™›@PÍåüs®?þ­&žû-]¿æÑØú†€¿ÙíuÝ/y¿àÖ¾ù$™'¿ÊŽ!%–ŠAGNbll?ïöïrêh?DyÍ
ð½Š??ÎÏb.uH?5®4g¯÷]?DZ˜=wé?:ñfü†Y?ï»
q¥L?€‡o£Ž~u?lE>õ?nÆi®‰Þ˜?tVÅó|ì?xƨ1>;Ò?ïLjiÞÊ?'úr\'A?ƒIÆEüé?xËøøâòÙ?‰"""CÆ?uÒi¸a "?ï¦2?}·Z­"Û?=À)9ŠÇ?Aa|b¢E?……{.¾g+?}…:¥!†?ïüWÖo|©?.†i'C,?-"YQ(ø?"Ó²C†[?,ïB¦b‰ì?"2£"³Ä?ïçiC™?c>÷Uò-å?Uåý´T?Sń~áO?[HgóèCC?YæfÚµ,Å?瑱N'*?oD´mG?t'ÿãsW?e~Îàò?vq¯[Öø?`IýVW҆?ïð™àç6?RZé©©˜?ƺL8°?'Ä'Ú¿?]ÒßJ"Å?QøÝˬAGN3FGL J1152.3-0841@qq_¿ƒ8.@I¶hÌÀ9(ÇôøÀ;"°Švæç¿ÝÆ Ò@""†g¹@Ž=Àâc¿æO&ŠÈ	]¿ær^E"_¿æç$˜`¿ßf¨ÎôL÷AGNfsrq?ïûEÏ©1M?AФ>íü?-ó'j诹?.*á'œ†?6×»œÝsŸ?<ùó0J?ﯸvËÛ®?¹'öKÓ?p+§Ñ¨B?o}™Š·?x˜ì5?{O~1Q?ï-Ç`Ò'Ö?†ÜIÌïá?'†džÆé?uõ""@rà?'á|€Zä?š
šÈ»?ï>û@¢?Œ´"]p"?^qœ×ÆÔ?[z1U'ƹ?–@'I»F?‹Kß綦?ïþLÞCÜh?#x‰KxÌô?h.{?Y'?uN?üšªÛ?$¢†6t?ïãñýýû?güWRBA?Y\5"Ìü?U#G[÷á?^ý©uÇÝ?a1îb'R?ï¨Z`¸k[?lXšõ•?ryìÓ?_JË :ê*?yXãx=ì?c'°®ix?ïßS%tŒ?b4»G6ï?9+íÛ¼ª:?.çöR5?m¾/H÷?aš:ïaA¤AGN3FGL J1153.4+4932@b0öÿ:Þ"@P=ÿ%¿­À8Aó‡K¹<À;–w§×Iþ?éCVqÚ@†@I~úï@A{P¿ãÅxãŸ)Ú¿å"ZíƒÈï¿ãIŸá‡D¿ìÁA_yAGNFSRQ?ïõþ¦lC?Q|•éÀ?MÝAíê?J|PI¢Ã?;M‡Ø¯Á?<3¤ýî??ïÃSPMäÿ?‡"¬UðÌ?kÓ`Âéñ4?ƒ»çºøY?pl§–Á?tk2•?î‡
Œ?•z)~ãçš?œ[eÄdz?¯W§ùÝ?'a@A ¢?†²Õµ³û?ïþ,—Hí–?>"¢»žn>óé5ÿ	»!?…ˆì¤L?*¹fc[½W?=TIsb?ï÷éOM?DiðÀߑ?I2ãò£ž?BôÚ&ÿÆ?,œ'²Ðu?&ípÛßL?ïéÇçµ±R?iNÄøܹï?SèÜc'?TÊöÒ½y3?X‡ czÊ?a·î'GÚ?îû¶l­[?åmAFÓ@?"ÇèB'M"?†DÊ3š€?‰'"Šà?€Ø8Šà3?ïÿ½…º(?sË@^>Î3©í¦ÁQ>ä…å
X>ývÆNü1¶?§Âýf+AGN3FGL J1153.4+4033@d`Ï‰@Rڀ¶–À:wŽF@À;ÙUËäo?ÍòÒ_*w@Ú[Ü®l?üF!_K??ïúGþÿ¿Ò'¯·µ…Ö¿ÒÑ;Ïíq;¿ÚÝx-Z£‡AGNfsrq?ïõoÒº'P?SÌñ?0?A±›[­?L²ÖÀ¨­?H×æå›?Dóˆ
ÿU?ïX'åqù?šþëüê&?…*Zæî?"õȊ©?"µ{¿—nÂ?‹W£µ9MÎ?î۝×ÁÈ?ŒI\¡^?ŽKuÅ
'û?'\~2™[	?•xQiaêí?"Z–gH®?í]äóÆG?¨>÷*:? €êö(qÖ?œšŸÓðW–?­‰6¼R÷·?¢[SµJ)c?ïø؛"wÁ?bë§ÃOãÕ?;L6ëË©Û?bŠJ–±?=îîô"N?>ó\ä¹ï9?ïÈ<¼3š?|E(°¥³.?k8v'€î?q^/ñïJî?l‹€¬®¹W?qM\8Áæµ?ïLReÊ×w?‡!Ï ü4?{h º4™?x†ßÀ‡?‹oýëˆÃ?"iÃ:'·?ï@í>˜}K?‡Kf•<;?ˆt	½#ã?xlLnÂz>?‡P¦œÈ‰W?€kRioPAGN3FGL J1153.7-2555@qðe¶™…@A"Œ_õ3À: öC¾›²À;à ɤ#`¿ÊF#.§@
ˆùyO!@9 4¾N?ìÕa¤h]¿è"ÍñÔ²ä¿Á7æÁj˜û¿ê8חAGNbcu?ïÃhܧ$6?w›©l€Ë?bNýÑíí?c•Ò¢í0?u$¤Šrç?r…A¥Á5	?ï2–-†ÿl?•Ákßeðd?Š½a¡ð?†öE­cnó?ˆÿð?²rÄÈ»S?ìøÝþ½#¦?¡cc¬Á¢I?©]e	;Š?™!bŽ£?§°ÜX?–±h&á¿n?íà&KÞ?£>«ó<Ð?"ÏÁÞWß?†Õ39—¯?¬ÊÎ$M­¬?¡kK²z…?ïè×÷ŖD?c€
¹Ìsò?PQ°Û*aÁ?K
EDL?]þ_‡Ë ?^ª_'?jê?ﵑ!Ùw3?z…øuÇ«C?s ó(¢Ôµ?q	–V–?r{ëQ}ç?qŠbr" ¬?îAÌ¢Ð2?šÇ¤¢iÕd?¡!Ô|s·ë?•ÉVƒkñ?•'ÂÆWä?Ž!>5'*‡?ï†Ê*õ»È?{Õ$÷¡z?r&Ûê׎Å?böXŒ^Á?…:<ÿ¨?w¥`iz¬"AGN3FGL J1154.0-3243@r²gÇ@<œûÿÀ? À91ÃÇkÀ;iEW"&?ï­qpì¸a@I¼ˆ†÷«@lÅßȧú¿Ü‰I±5'æ¿áˆý&~;g¿Ü@Ö²÷¿æ¾üHÕÆAGNbcu?îªnD1¼?¡¹²yöwQ?™Àõô¦j?™©+lq@«?ñF¢Ó^t?Ž¢ô±=0?èc@9+ß?Â@›¦ o?ŶàÅZÆ(?½£ÿŸ5?±x<«ñ¤·?µé§'?ì€éäF;?¢ô÷Ɇ¹q?¬Oƚa?™¦2%¹oo?«ÙT"ˆ¶é?–«gãÂ?ãbNÅ¡Ì?µ4P,§Î?Êz¥¼×P"?´++ƞ?Çü.Þ(¯?°[¥%­¨?ï~CE‹5º?‰¶¤&c?ƒ×þH¸³?ŽÏQ9–?zÔ­;¯?u²™6ɝõ?ìœÆ9 *?´6'1³†?³9hâ?°Í¢ŸL—û?ŸêYå‰J?¢%t*_ª)?îJ4Å74Ó?–wœ¿tç·?D²&V¢?Œ/väXœ´?™uX¬xó?‰œw<?éh
1¹,ÿ?£ßlÍÛ?·_Ðþ"L? J}~5?®¡­¨.Ò?•Õ¼~"AGN3FGL J1154.2-0010@qå¿­)™@M¶xßå®EÀ9ÜW?öÀ;r¤Þq9ÿÀ|v4ÐR@¯9"õjÑ?úð ¦=¿åô"½Ö¿ÝÜSH¿Ô÷"}~c'?£ÀÌó&JAGNbll?ïû¨èõý?@Êahà?®âµ·¯?Û¾PÖ?;M`"?>Ú2´Zב?ï̸¹"Š?{Ñ¡#Ïޒ?eµF²7¾g?k@·&† B?m'·ÏMÿ<?rþ´àε¦?ïm
LÍ@Ä?ƒ¨€ÌH	…?€)Öîܽ–?}*¶û'Ò'?"'Õçv?y>"'è?ïóD"ë›?Vãg_áð&> ÏáNC"ø>­…ö`f?Xÿ]WÆÓË?Vâ¾Æº1?ïým€®]˜?+-CÚis|?ã¾2pT?4µ€Ù?,6jN|È4?$´¾ð¥çA?ïê>"Rr?bŒbxç?SÅQS'ÍÅ?SH‹d7?W<10'ÿ°?V`xµo?ï±*]²ÉÓ?|%²G_—ð?sëI…Ÿ,§?wíÁSçǜ?s‡°2?o´3Š±H\?ïýµ9ª"?*Þô£z~>|Öøu+9>ˆÐÂ'Öì?2Tq ]qÓ?*®lݺÓAGN3FGL J1154.3+6023@`é¦Þüz:@K¬ºAn_À9‹æYeÌãÀ;Ã^Zÿ*?â,š-±@{ÅËÑ¥$@AÚ?üð+¿Ö\Ù²ìÆ¿èy˜㳑¿ìšý‹ K~¿å$r3µJ`AGNfsrq?ïû£
Aރ??ü4*4˜B?9­ÕrÊ|?;p/¨Ö'?#©þ?ž²i?'ˆõ˜"bW?粒Þ;<Ë?"3l¬
?s3î¹@†ã?v¦ŒŒ¹ä?xï"Eý˪?~ŠQ?î5AZ4Ì2?›*^H@Ó³?ŸÍ@¹NWá?–!Ão—?™Š"!â?/Š`ð?ï+ä2L¶ð?'²€ZÚ?ƒÍq3•¢?€½êã4‹?œëøO÷(?:I6†£?ïý¨X4…ª?0°º'ÝE?(i,°§C?+èG©v?"ñ;ªò¦?Ä5ÆÀW?ïào>QIt?lÆ6Èæ"?Z i\Zþ?Vll«ø?b@ŒÉÉ?gÁ…'f?îó]Eç|?"ûÓlñgX?"[×y:ü?."Íì?ŒqY}[?†eH*Òk¼?ïßb"Àª¼?iI0	Wùƒ?^¾íãÔ?P#ÉÜùî?a>lŸ(
s?e|w#&AGN3FGL J1155.4-3417@rEߨq¤@;(Ràw¤|À:Š…=ÂÀ;š®]uüÜ?ÚÃèNÕÈk@gD¡D³¹?õ]ß>>?ï†	‰ÍI¿ä–.ÙÃfƒ?¯zH<ý¿ÂxrÜ°3~AGNbcu?ï¨ë|míL?‹Müò‹K™?@Iúâù?C{Þ{ζ2?"À-õ®.?Šû… RX?ï™ÇǙ ?"ê™w›ÿ?tFЂd¢Û?'ëæ•D¡?/Ë ®?‡­'2Lm?îYDgÁÝ?"™¯îd?—Oõ±~"ï?Ž¤ƒÇ9(Ú?‡}[w)j?Œ
¾š»õ½?í£Û=—©ï?©ë¿T‰Ý?j
ä	ß?yo>[ð=®?²Ò|nw?©¿þÊO/?ïÊîE˜e'?›_¨&è0²?=Z…!¼>ò?D'ݹÚ$?x³4÷‹Ã¿?›/ˆC¼Ñ?ïØoÓU0?sG]2¿?_Ýç…?"w?XY‹!´Ã/?hœrJþ?oñ,þÖ?îÂ\Ä&5?™SÐ8qs{?•~6N·Y?"Êc('î/?'61*Êwì?‰U¬í¤×½?ïsû"rÍ?"È"%]Ôê?iûarÿ,?eû!Öê?Œ¼ÜSxY?'Ø]RAGN3FGL J1155.9+6136@`Ʀ?šIÃ@K%v¹ÃÀ:Ïÿt¿Å}À;÷û'Ü5ö?áõûÏS@8H‡®4±?úVÿn4¼¿íÕĘ©bB?ïÛ ±•'´?®ÅEÞ M­¿àÐ3xl<AGNbll?ï÷v@Ûp?LI{´âF?;X\‰Fr?@½#{}×?Dy´ü¨‰?Bcò®M<,?ð'ßn?¨}pY‰}?œe½Ù*?¢QtþäßÚ?'ž\Øæ9?"u	¹´ŽŠ?îÞs¥‹Œ³?Ž¼2àLèX?'5ùbâ5Z?ŠNmìژÄ?'û'ïÐB?}•~	??î°?¨'‰É±©?§z1Ț¦?¦ûÈN=È?5œ÷´ò?Qw"uÃE?ïúy¥ªÁW?>"¯ÞÑx2?,ÄFšGF?&Ên›
ªJ?=ÐÏ¡Å°š?8E'æy}?ï¢ÆS}Ö?"vCÕu?{ÀJŠÌ"?|BÀWëÃ?s"Pc®?sóÁ&k¶?ïhõ~`œè?F4ÿ{tº?d@Cž?zקU?"3<U	^†?qS°F{YÔ?ï:Ý؟?Š§"9ô?•|®ˆ¤Ó?ˆ]2*â'6?jvo亍?eÖ"vûq"AGN3FGL J1156.7-2250@qìò?î,™@C'.ÿÇËÜÀ:='¡}"À;¢£Ìhú?à`ðúP@
/FB¯}?þ=~`X/l?ï¶z'A&¿äQƒ¯½¿ÙumKv»¿Â£¼y© AGNbcu?ïíãánøå?W4é'»A?C¦0H1V?Cãã=¦­?Z´j'	B?Rtâɚ—?ï9¼—Ô?'¹´Ö±´?yB
ÇÈ@Í?"á"harŸ?€ì8üŒŠ?ŠÎ'
?îædˇ?‡˜Ljó¸?‹8ÒY~¡q?{+P7f?•'"ã7¢x?™N"=Ô?íB¯ˆÕbY?§gYø¼6I?‡³>V3¾?'i_1lH?²ôíD²$?¦ ™nÃD?ïø3kDû?CŠojÌ=Ý?3ïøÄ~Ô·?1ºÇÓF?E:UŒd\À?<"H,XÐò?ïÕaâ%Ø	?u:Ý\v'l?dšpÍQ;?hšõúœ?f~ƒ/¡5¡?l2«µcAH?ïwöQ‰@?vLEBøI?}O2›õE½?o@¦ql÷t?ƒZÒ]<ï?iށ£)J‡?ïXF÷úç¬?ŠKrú[kÛ?xn¤fË=?zÉõYÄO?·4#
n?ƒŒmª"]AGN3FGL J1158.8+0941@p­ÿ'+¿@Q&^è¬À9•,D+¨ûÀ;˜È¡ÄáFÀ0°ÿç¬L@«=ø9à@R"`R%<¿Ûiís¡Ÿ¿âì3ˆ©Ão¿à©wÍA¿Ò;'§%ãAGNbll?ïü¡* ~¿?,3BÏNi"? *ùßL""?óhq¹³0?2á0$4ÞÁ?%H±¶ëƒ?ïÅßIôb4?€?…Î ?i<&¥ôÚR?oÌÂ1Y'†?prG·£ì–?uCL*Üê«?ï†(…Ó-?u.M«"K?w¶éÇÀ…?g•"gç ‡?'ò +,}?n¿¶ýÃ:Ù?ïßyo$Œ?lv|™­µ>ø'*?ub?1($j?p*ÆUKûC?llu½Pç?ïýêt†d?ÖûòŠIH?x–˜P×°?
ªy»ø+?%j»Ë¥?ÌJ/‰ÃË?ïé/È*â¾?fïÓPŒAè?TO"ÖÑßa?Tj~Œ—?YPÚ¡îE!?`¥Ï4i"È?ï'€N!ª?a‰ªð gh?i{"û8Û=?Pï¨Øp€Ü?qù}[R½Ž?Z€%›Ñ}?ïú»Lò¡ô?@ÄÆÚûs>ÄÂ.rÍë/>Æ®T$³£"?DþkÎ;?@½ç×=1ÅAGN3FGL J1158.9+0818@p°ñŸŒ¨@PÜäÀ™,À:§ÎçY@À;ð?HkÈ¿¾ç­xɕ`@¶õlÿÜ?ýéeŸA#a¿ê|Aâx…£¿Óûãl˜Ò¿ÅwKu
7¿Ù­/}ñóMAGNbcu?ïòÍNÊ4ä?^ø0QÚ#?<ã!†©"'?A›"ʲ'ó?S,šO½{£?\ LÑàÍ?ï«|În8?'òP"íãH?s0#û›¥?tj.4ÚFð?wҘš<k?zÙ1'ÙŒ—?î–=ðŒ«±?•Ðuå ?ƒF÷ù‡Ô?u¯ô+5åÌ?¡Êbû}m?•«×Žæšü?ïw_ø¹Õ?ƒi£ò?dˆ€Øݛ4?g3ø
ðéð?á'6?°g›­‹?ïúHXçÖF?G +\
C?(…¥Ôöƒ?&°?µ7ð?@½3RÃì[?E"Ý=<(?ïã±!9zd?hžÍÇÿÍ?Y¿¦å¯·0?Yi¥×³º;?^Þ(ŒÐV?aÄë¹ðNÏ?ï30àâGL?ŠHw
ÄM?Hô@$L?x¯'þ%O:?'ǦÏ
Š`?‡Hï‰Ç¢?ïàÚ·WUã?^S©xyF?V5aÃáÕ?IÆpiDa§?d
——£æ?W´š^$AGN3FGL J1159.2-2141@qòs?Èlì@CÊÍ_™Ã‹À8Û¼¸''íÀ;>£
¶¡è?×Ò8ôŠ£T@Cˆ™A/@â矶ê¿âóâhž¼¿æ¡y™ÁT¿æiùB÷vo¿àôÓ;YÏAGNfsrq?ïüj¢hÓ²?-öғ|_Ã?(–-3Äú? ¤b•(?0_ÖÌ"¾?$Ø`YÞ×½?ï¯fw?Ž{œg?o¨¥Ô"?lïpר?x« Œk¹?‹G	kóõÚ?ïXc/
•Á?~m€íî^?ÅJ©DÓ?mUPÜìˊ?ŠŽà! 3?uؗ‡KÞ?ïrxù™'?…Šå­¶Š€?Sµõ®b?Q$±­db?uk¸Pb?…$DÄ?ïþˆ¿ÜI?ú'>Àyg?K€À–Lù?XgàÖÑ?œ¡ÊY'?"NŽ¿GÐ?ïãÑ¡¦a?h•¹0©é8?WQÛuú?Ràё'žÖ?`fQÐM¦ú?cUr‡ØÏ?ï­"½Q?kSƲä?rG"R-Ðm?chR'ì?w/Ûm'%?_èg.£±"?ïâY*á?`փ%U!_?A‡½bL1V?1ÈT´ŒŠû?i›·Iz	?_ÿà¶ËoAGN3FGL J1159.3-2226@qö`RP/@Cma .QÀ8…ž8dË\À;ÍèU¿O?ñ_ß0§'¬@&æÓE7@ùSŸQí¿å\¯:ëŽY¿äZDiÁ¿äªP!Å;x¿êŽã4îVAGNbcu?ïÕÈ	!D|?oçû·#ù?rÏkî$³?lÐÒ×-ò?HÑaâ	?GÇ­~ï?ï'Ã÷'œ?†°žT$«—?wøüEø?tÄU½FQ?~¥Ý(?»AZûe?ícüg!ÕÆ?¤b¬èê?«Öûˆx¿A? p"×V?›Ò|ô½?.IrѲ?în–iʅ0?™‡{A¼NU?ˆÎŽ
·]+?•‷L?¢âõ۞Rº?–Ü©ä•kb?ïîZ±@C?Z¿t½ó?_f%tòŽ?X뼿´?2$'£'Òm?/j
°_]q?ï΀#¯e;?q¦n|%
­?g-°`ß)£?_{të¼]ˆ?jR+úºZ×?j'?UDóØ?îárãÄ­f?'³L¾·š½?˜—¡ƒ;Z?³¢îÒ½?†t^"Ó?ygBP|Û ?ï"C[–?y%,Ðd§5?zIJ͡KÓ?gÐw{ˆsÄ?ŒÆÐq
œ?t¢~Ё–zAGN3FGL J1159.5+2914@hî?àH@S—úÀ%À75#Â|ç²À:ؽØ=CW?÷¿·e‡n@E|^Jc&@éý¿]ù¿à7Æíî8¿ã"<b3¿äÂBÀ
¿äcåj}wOAGNfsrq?ïø˜(fŒ¸?BjÍé2a?,À¬±©h-?#¯£«h¿?Fo2I±:	?@ÔÉzú{?ïŸî»ñ˜?—FÑGF?É?gˆ~f|ԙ?nO	­ô´Ž?'"1z˜ÄÕ?–Tiãö?ï6 Eã?ŒÃÿV‰dó?ˆêÇ.‰H?ƒwI£8/?Š?ÃPn¥?ƒEÇ^¶é?ïöQ»‰ƒw?`ädØ?œ?
'$¶8?,LöïÞ?RoôkäŠó?_šj?ïûwàaT.?7b»ï½ø»?)Ï`ñ‡?!Õ\½P­§?7Y{tŽ°Œ?1Ã(N?Ù?ïÝz»CH»?€W${ ºi?SEҗ›ùT?SrSÆÜáØ?hâ[j
?~Ã+«ÚÚÇ?ïa»®ŽÀš?‡ÐOR·ô?"ZF
ӗµ?€³ œäB?ƒ6ÎY{º?q%Nq'?ïþŽ«©çp?1J7fØÏ>õ˜õÜôæ?ø¾®e|?$b#î_W?1É0AGN3FGL J1200.8+1228@pX: WŽ\@QÊ9`~TÀ:ªŠ'¥aÀ;Ò7yê¿Äf!‹Ú­û@GðÂJgØ@üµ?½Z>¿ãɵî¹Ü…¿Úôê-ðÖ¿èäXòµi¯¿Ò €³2ŒAGNbcu?ﺡ\è?àtQ
I?p*²[1~þ?tÀpÂc¨ù?r•}!¤Á?vïÏx|'>?ïš÷ÏÒ24?‰§†v?wh¢sbnN?€†u¿ŸX?{u«Ã‡¾?€6Ü#A¥?î\Ø¿Z"—?–±YÔ²ŸO?˜i-[¦ñ{?ŠÂ,úÁ'?›ûººÀI ?ˆðþƒß2?îáSóB?•¡ v˜
?‡.ôwE7Á?‹
Žw2?˜8›EùÛå?2"öÎp>?ïáž-ێ?–ßGç"?c›×Š¨â?––Kc
#?U‹õ`ёW?a¼Ä(Oà¬?ïߥTÏ?l×óø"éc?^i˝/Ì?aÑӀEä©?a&î†Á?aqQé4H?ïU÷Qké™?€¢Jtų?…¾—	Y`"?wP:ªžÃ0?"Ô¬ÚE?o¨ŸÇ2:"?ïÐåÆBïê?lÇåž;0?\…Õ?Ø $?Q«&Ø.œJ?pk§o¥gI?h4¼" [#AGN3FGL J1200.9+2010@n)<ßï¿@@S!ãŸâˆ÷À:»˜¢úÀ;Ô O*à~¿øâZ=8DÀ@;ªv`¯m@1Œ` ÿ"¿æ0o<+ˆ¿ê?äߓ#¿àvºól¯è¿ïÿåÊ/õ¢AGNbcu?ï_ "DrÌ?¨ì»ò¸Xq?GgLœ´L?Q)–'0?"Pµ{+??¨¼JQ:Î?ï‹v''R?‹È8–Þú?x:•ßo ¨?|›h1/ã?+AY?'ýÇnNŸC?ìÿÌ^ÆgŒ?§Lž¡é?œ¯–qv.?Šò¡ÊIø?°ûñ$žY˜?¥8{x.U?ï`­v4(•?Ž—c‹`?hÞj"+"?qÙTrXš?ÎqQÑÚ?‹{îÖ€K?ïŸҘ¾¨?'î"KŒl÷?Aåqíõ'*?TmØ׏K÷?|shn/³Ï?'ðÐjÄ¢?ïÜ+§£?nU²Fá&P?^zãTu£?[
û;Û-z?d–æµ öª?f®îoPÇ ?îDW'%«-?œ)ñÇ×:Q?•ÜË1<(?…¸ñVL›m? Ì'õ@¡?—´¬I¾r¾?ïæ~Ážh?c³€êR?2"ððåi˜?3'¯d=}?g¦ã1ÿ³ª?c$@³mº÷AGN3FGL J1203.1+6029@`­ñ¾ôœõ@KÑm`U«-À9qɕà§À;Ô#ú±¦¿ø4€z¹¯@²:)Çy§@ªþ¢Lœ¿é<*Fê9¿ÞíÆw'¿á»qä'¿ç™Ä»¹ÞAGNbll?ïÝ	ÀÖ[?kØgN߇H?cZ"¤{ð?bö–‡±Þ·?_8ÕwSé?['ÞžU]?d4[?ŠÖ÷¡vW¬?w½G_£F?}{‡Ï†O?{þ0~ÄGj?€{iåÅ>Õ?îœ4² añ?•A½ù"?÷hE¨o?"#§!´%?›'fKRS?W"«Åy?ïa^díÈù?À$Ø-|[?g
ü¼3a?p'*í·"?ô;-f?Š¡mªPÁ§?ïö
a×$X?PT
×F X?HÄã­Ì)"?Hñrk¨Õ­?>*z4¨Ì?<*ƒf¥ ù?ïßÎÉɄ?q£o±•Æ?^t°lt?fe;œõ+?`öÝÃÈGÔ?bÃØwDîé?ïƒRQJdA?|ë>ÔÞ]~?{ékÊñƒÐ?qÛgÝC?6µÃv¯Û?t½ý/ÏÔ$?ïç˜$EüÜ?bztZç°?,xÊ&"?1qM9‡[?f O5³CK?bãûSÿAGN3FGL J1203.2+3847@dààëgÃ@R¥ïß÷KüÀ:k'öjÀ<q/îU¿üÐÚ8M´@fÝ°õ«¾@m!¬ˆŠ¿ãAÿÞЎ¿în-{°?ݯ8gOšr¿ïÿöõ;ŽAGNbll?ë¢Ýƒºpe?ÍZ3Ð7?›K׫h?³k{¸§	?¼ù$P?ʞÎ%¬%Ò?ïh1]	4?Ÿ=¿¢C––?ƒ½9~ø=Ê?–O)8'?'6'b6Q.?‡æó!qÖ?ç\~áK?´X]wõòð?··Žß"Éú?¤°×rÉõM?Æ´(4ÁA˜?´"	§$¢?ï|š²jÃ:?˜þ¯°Í¶Ù?FÔɛ-~?bý'"+é*?lÛ³¼Ó?˜­ŠFc"?ëuä'B;?щoÙ	y¯?¤èî= L?½I"3(Ky?¼ÿÙ»-ú?Íë'ÿ~Œ?ïÈQ}ÿ'Ð?±Rß%2ø?n¸¼eÉ¢ê?‰j§÷Qò?hõÅÇþd}?s¯']¯Ž?éÀö²EÚL?¬IJ–¨?´¢\?¢*MßÆtz?½ð¨_+'?¨äP¹5S:?ïî/Tù£è?gbk‹èv¹?%ø¶çU×?8\Á!ð!R?`qZ–×ü?f5žuàý'AGN3FGL J1203.5-3925@rO@ €@6ƒËßgDÀ:2.¸z/qÀ;—øö ƒ-¿½ÄfÑ	6N@
"Z"
kê?ú7Ó@"TŽ?ì;dÐ9=ä?ïš[ÓæF›¿æÐ3¶Xu?¢¥½‹³ŸLAGNbcu?ï®Ê'3??"Ýžћ?dß¾	ÇQ?gtEµ^v¤?~*à §Ÿ?'Î	þÓz?ïa!ćB?¢ÓGaÔ¶?~ö'í…í?… §5%¶$?ˆ<MwÒÖn?|VÇõ¾?íþX*c€Ù?˜{¦Ä™ZV?žðÂý‡3?'"žcÎs¥? ¢ÜØ?Ž7YÜ¥?íÅ«Û2º?°BF¶…©?¢uú%rÌ?­î}]º•?¡/H*ӑ?¡|ÄJJ?ïëQj´\q?g£xþ1?G¡v¦O#?J$Ÿ9Òú?]Œo—l°?dÍE•ÐÕ"?ï̽÷"C?'þÓP8Ãf?g(jHt?s6Бv¦?l&n4ì¿?zó¢‹È"?îþèƨp?Ž‡Ô"$6W?'íu²áH˜?ˆE-7ôl?Œ¡Úe#¶¸?}‰ž|êб?ï­Þm'±v?Îå}±Å?bÛ%±9¦C?^šÁ?£6[Õ²?|<×\AGN3FGL J1203.9-6243@r˜n «†¿ÖªƒÉbÏÀ7Û5÷2ÑäÀ:*Eå"T?ü$NÂÜ@Sjøœ^p@.jÑ¿á'YŸX…¿åÇVVVu¿çP§'«"¿î'+'uPSRpsr?pU7įH`?l;+Ù±dw?Óü1ó?È*M—ž¨Þ?åá=p^?È<Eãö?a.ªÈv	?t'Ðqå?Ø{Ùèò¥Ø?½úWbL?ã°ä`´˜?¾fÄ|"›Ë?´?CÉVÁE?£§bÛDžs?×[0nCÛ?·–FÙð?áÊOÁ^Z?º–¡ÏjƒN?¦¶RˆŸ1š?™£Î¶7Þ3?ØÑ<;M;¦?¶¸ ÒºK?â+ü¹Š¶ä?¸ØUùfØ?o'ÖðK\?s™›Kè7??ÎóÅÓÎ
?Æ+—'ÏQâ?è$ú49?ÆDy-à°Q?yÜ^áœô?ŽÅö_k?Þ`0*Ùâ#?º+›à××Ô?àÊ1Ö«?»¡ŸP×wº?ÂM³ßbs	?©Ü¾xÊaÑ?ÖùÖ:‰¾°?³¢D	B"'?ßßOÕÅË?·7MjF8×?­¤Ôc® ô?¢Oy(?ÝÖÄôL~Å?®Cï&À"k?Þt « œ?²ºci5OTHER3FGL J1204.0+1144@pŒy¿ß~€@QÀ»À5ÖÀ9°ÙQÀ;›¢ø½ì_¿ÒR¢v?«@%²A±%?þ	'€J¾¿çVöو'¿ÖßŠ§ä5¿×tæY1¿àœ²ßwªAGNbll?ïûB'¨'?9W£1Hí?,˜Ž'ÙV?#î›6ŠæÀ?7Ÿ*²Jè&?3'úß7w¾?ﶴ»š0©?}çrÒ?mÌ+3T× ?nxæøp_Q?u¿Œ®ŠÓ"?y©;îÅÁ?ïsyš «?z9
Œò©m?},ì§pU?q6û+'O'?"¥«V͚'?mŒÏþVo?ïyQ.w?iÿ5rX-?\WSùÒ>|?VƒV@'[+?Ž Ó¿m.P?€€sù?ïþ;ÎÑùv?ô¥aÇá;?Íl®ÁÕ?
³àþz/?¸»ÇG`?4avÞÀ@?ïãüƒ–?gÖ|sÏøª?XŽ«×ò3P?V>2'k¥?_xL˜æœ?`ôòŸá›?ï³*‡Æü?i·û+e%?qÅ!¾[çÓ?d¶›$?t¥š{8Qø?W/=[[j'?ïàÇzÂ-?_¿r
"\?I¬Í´´?6ÕpõÐÞ?ix24~¹?^	w!åAGN3FGL J1204.3-0708@q­µ?|í'@Jño`
+ÓÀ9böo]†À;BöÕ®?×ýµ(/@ý4XÍ °?ýÇz Z(¿å0–Ý@|¿ÓP–ñH­¿Ô(SÜ '¿âV[À+dïAGNbll?ïí¥_þöÉ?X@‹%¯‡X?W³—&¹±t?R=R?l?JRÅ,Pš?EØ2"éÆ)?ï=ï9ê»?•ú)"ú[?‡?«â±?‰r`ãi?‰Dˆa#?ÉÙ¼ðñ?îÊS€…¡?'SÉM2Û?'¥Z,¯&?ˆßU‡é:c?"é³2S±?…ßÙ]Ùa?ìIè"àø?¥T3mqœ?œ`ÏnTÖÎ?'óÿägÇ?¸%|âwێ?£^Ý¿ª?ïõz\@ë?OŸL_v4?K9*W?G¨…ë	dÐ?>	#jíLˆ?9•›?	?ï¾#†íÅk?z¼	—?pËQ²A?p@»Óž'?p^q"¶p?r\–ô6?ï]²ns
?ƒd'Èøš?…ãü9-†?7þ¯€C?'¯hP\÷ð?oûAuZeø?‹j?‰­ûtê?'ËKh?KÉ?xÂ3û´Þ›?›ÀÃ5;¤†?"\?*j;AGN3FGL J1205.4+0412@q5»à~í@P&3`<ÎÀ:.
¦L/ƒÀ;͒ûç2?œ9>ce@ ä}m"@!=ŸÈ²·¿ì/£sžD¿Éë17–«d¿î?`Ɯæ¿ïÿ¹‰¬š0AGNfsrq?ïDŒtˌŽ?š/z%Ôß?–¢×/ý?™R³e¤rÜ?VŒèÔêÑc?k¬°ž\?ëöHh|É?½­T¢N?¶YýßÇÖ?¶´½]<H?£ç~a¬X¾?§IHjÊF?éð%"pL?®®Ñq¾_?Âr
Ö
?¬1D&¬?§5;ˆ,¹æ?•úu½ÌrÃ?ãÌI€bÍ?ÅÕãXÌÂ2?ÕÐêWúS?Æê³´ð.ž?¤´;"Žo?žXK-–_T?ï^O18®?˜ÞW04ót?'ù†¹ùþ?˜f¢¯"·?SÉ2s¥«)?dvXPø?ïøIì÷Ô?˜Å½Ÿ|??'uÛ6b‹½?'|qõ^é?…7üór?…?Ux7µ?ëqK®ej?¨"<?½´3g¥DŒ?§
/+W?Ú?›
hä¿ž?Œeh^-ö?î)p{q? }B–•'«?§I]xË?ž4Ým´?‰žÕ÷ ø?ˆ+=B*-AGN3FGL J1205.8-2636@r'=ÀTïF@A"ÌÀ7"À9+v2ŒDÀ;v¢À‰Èk?ÒnKa49@}ýîØ»C@S.Ÿz¯¿ä[8€$'¨¿çÒlÁ<‡¿ç'"±UÖ¿à<|+AGNfsrq?ïüNëž+?4S7(/j[?$¡	°Æò?$ïœR‰×?3@×áZ¯ ?.ðöî1k?ïŒVÿ¯çÓ?Y‡Ùô@?víù6ôô?twY-ç?sC{KA?ŠŸYòÆ£Á?ïMhÑ*?"lŸ¼à?¦ªˆ&S?qV€zè?ŒÒ§ƒòP[?v¯Æ…Ο*?ît%|nîÿ?–ÊxÄè0?~+÷'槊?wë·Ï´»?¤ø)Bª°©?–25¢ÈC0?ïþ++ÒÁ®?*<^[íb?K‹vÄä?äæڝ۾? §z2W@?%Eâád?ïØxª5É?nÝ×þÛp?a6ç•Ìj²?ZM½öŒ¹?fPn*˝²?iš5"½9?ï¨TªÒ&(?tÇ]Œ¸¸?sÛëuôÁ»?q¯»Á ?wù¿2&6)?d°tÊ}Í@?ï®ï¡Zz—?sD¢†ÿk?cšåç€xP?OxPàà?~º¼p0"?qÌÕïªÚAGN3FGL J1207.2-5052@r}©ß—ª¬@&ÉÁ?ÐÐhÀ9É:qÀ;{ö?ŒÝÉ?õÛ£g"Îâ@gwñB"@#à ¼Ž?Üu@å£]¿×K".ùñ&¿åÂHù꽿îaÓZGAPSRpsr?ÅrÑhà6?À¬S°<¬?êa°ìhì?Ág)k¯?"ßË_ÂæÎ?'<½È
z†?Ó ßÖaBˆ?NjBÖ`Á®?܅)?iwh?Å)žšgþ?ϳí֐Mž?ŋçâe?Ò¶¨úpÛ?¹t,êZ+?ㅜç×À?¹õô莎?¸øtØZy½?q:2‰r¹?Ö3êI·M?´‹Ä?-¿
?áX/)õX?¸ƒ·«¹'ï?¼n݋êb?«ÊÐÞªDã?ÐåÐQ¿?ÆKøå
?ç Ñ?•?Æ}ó9·Ëx?‹(ãø-:Û?"Zç¦C«c?މ1N<à?ƺwòsó?×K Wìِ?ŸI˔Ø?ÄW¶ï¯"œ?½É‹—ÖÔk?áFeÑ&^ö?²Ý¬§Ð?ÙAx/çyK?²C‹;Äp?°Æð¶Á/¦?•à¨Ân‰|?ã¾ãÜon?­Cì.‹‹?Õ5\gMÛÅ?ªá;à$D?ªfßë}ù?›a±ãÌÊrMIXED3FGL J1207.6-4537@ro@OÂ@0Õ€ÐtøÀ:4\÷QÜÀ;´²$ªÚ?õ}h%-a@Gý™Heõ@æùÿ_ò¿ç5§«uª¿¯ÃO`Þ¿âyaÅÇÚ¿ïÿõ³¶YAGNbcu?®ß›"fF'?µ1Ö/lÂ0?韼;7ó?Élåd%ø?ÁÉ(0(oh?ńNj«€ˆ?¥L%Z?µªmNª6?ëE?¨óë?Åo™
R"L?»RóÂáx?Àe	º=þé?ÑU¨­L˜¤?³×Aú3?ân?æA_h?¹yÍ^îV?Û¯aQ?¬‹èøn¿?Ã\‰´°\?²')éÍ'?ésn€¹	?¶öÞ©z)•?«Vø¶êË+? æNÝk}?§'£ Áqž?³Sxûxã•?虿‰ÔQ?ΜU•:?Ç´˜òïe?Ë֗ÖÙ¦?¼t}'Œk?ÅC‰¦¡-Ñ?èÊlW8˜o?˙o°ÅÇ?½œ(È©°?¼E×KgÍ?ÝÙZ"Ž+–?²ŽBÓ9™?ÚG•P§I?³kt.…ao?¿|A€91‹?¦'¿Kï?ÓhMh…?±yÔòüœ?åb\0'~Ë?²¾ÍÑF¾‡?3E&ФH?ŒNaD»VMIXED3FGL J1207.6-2232@r¸_.Q@C›ãø¶À9´ýµ¢äœÀ;Œ27Š±¿ád"†Ò@ñ3¼Æ@™@ ¦n¿â¦-QØöã¿éYA}h©¿éÜ ï'¯`¿ÛÉÀ¤õAGNbcu?ïʒ:ö ?uÕ¯gÀ½M?ZüË%®ix?YT7¶Æí?s÷…™õ"?sL§=f%ð?ï|W—Ÿ!!?–ük)?~2&VêÞ?‡:Ìl¿?Ñ$zžX?Ž·M7*ž?íü"Uv˜Ò?˜YÛ6É ?˜ßú¡ÓA4?Œö<j'Î?£ÆÍZ@‡<?2Œ·ajN?îZ"ÆÜüM?—'÷]¥M?uÌ9ë8g?tNƒrjF?§½Z
"àœ?–™ä™Òa}?ïñmØŽ'?V½M€ùÔ?A1Bk[U?@>N‹R1?T‹Ã³ï"L?R/K¿Œ˜?ïÕOiìû
?tfª"mÚ?b ;–~9?bŠ÷ùIû?h|˜5¥+?oŠ±ßŠŽ?ïC‰´–—~?€ÞÖÞø46?†ABD½$?{úí0ïZò?ˆÜP‡Þ¯n?q+Yóå‰?ïªaÄ]?u4F"Ã,ï?PþèEÖ¦N?@ȊŽØ!l?ƒGÃ-$Çÿ?t"µE—oæAGN3FGL J1208.2-7810c@rÊhŸÆÚEÀ.ùûg¿,À:7jÒñ²À; Ôký¿ó˜Õ¿9¼9@1<6½|@*A`y£¿èþv§kF¿ãOL÷¿ØuEWHw¿à©9c'»HAGNbcu ?ïë•0©@?^šu3I2Ã?/J¯ÕJW%?)'ýêN?c¿Où%?\՘\‡‡J?ïNjÀ¬ò¬?'ÿ9흸ô?t÷`ÝØ?uÉô ^U?ôϺÜ
?Ï	XT'?î{#ê7c;?‹ÚppÍ¿Þ?ïä%šHŠ?x»÷{f? ÑÈS#:-?…ƒÉn`•H?îÆ'Nû]?P£iM·É?C(r¦c\?Dð[…`Ô?£Pí±³f«?062$?ï÷}Òï"?Fó†ÊvU?"m®S¡¯É?ö—èGÛ®?Mn]Z¹)8?Ey¿'Ü;ì?ïÉùÖLÂ?xï-¡¤?Z'icà;ø?X{^nÁ?tbâ*³"?t?yUÁÿp?ïeÈ£P?r?û#k?|ÉX]>ˆ?apžÙp?ˆW¡›~r¸?ji…éÝ(Ž?ïºuKö?gãÊõ'ê?,‹fÿ?!g³K°Û?
ÈlÖ?g‰¿'7æÅAGN3FGL J1208.7+5442@`úMÓØ@N«"ßöu=À8rS±À;ÃÉfæ¾æ?çĝúZ\@{´+k>@X˜ÀUÆ¿äúÛùî÷x¿æá^‡IàÊ¿ç^Çζ0ÿ¿ïÿâóÍ3AGNfsrq?ïùÂa—}=?F7@íú?0bª±¯Þ?+ùOûàO?@Å$äÈ5s?C°•Mˆã?ï±0hõÚ/?ˆ´£`Aß?s¿WEät?ƒŸù¥dÎ?s¨.6*?vÈà¸HҞ?îƤNÔNv?'ßjZÓ{?•Y¸+§?‰SOi Š?'Òat)Áœ?‡-·âô›7?ï×sì?z>kŸ-&?]ì"ÿ.0ƒ?jøÖ?¼?i–¡µ!€r?t"Kcá'á?ïûò,æŠ?9E&ÜRó¸?-y"Î^?)[æ$y?1äá—Åí?1"&K=-?ïáÂf'¸g?nM®à'L?[œlÐíQª?Y¬é<»M?`oc7wX"?ebÌ|ê'?ï) "céx?‡#9eÞHy?43ÿ¯ú¹?~Íÿ÷rh?†ƒ¦ãæ;?~á¶5«?ïúóé=¾?P×<Ä;s?1ߕպü¹?AƟ§å ?6˜P¢]?I'
4	AGN3FGL J1209.1-5224@r†o€Uûµ@#܅_û¾'À9ùS‰XÀ;Œ¿Ígý¿öGþ3¢ï@
PëTø@Òc`¢'!¿éË"'È¿ç‰N'«?´¿Ý9iMM¿äø"PŒàNOTHERspp?ïÉá\É&?xú_ÿz0?Y/¬•E´,?YÍÓ¬Éå?tÃfpœ%2?uTåѨÄ"?ïTt§Øݸ?˜ÑŸ#ÚY?tGAªf½Ç?ƒá|
?ú?_š˜'Ë"?•S~õVîI?î"âül«-?•EQÞ©?"KÚTÒ?~~­ \[i?¤+ã2¿ÅÓ?¨´]¢ð?ïW­°?‹ó‡)]$&?EP[H…?E‹Ò "²F?ÌIå¿Fƒ?‹ŸwYFÐñ?ïò,Qäñ~?ZÑ^Î2Ч??ÀÁñÖЭ?<LV/§?S·+þ ¼?UüÿȊ6g?ï̦/eY‡?zr™r¨Ï"?[·eq—?V³¼T·k×?r¿&èçÕ?w™ <&r?ïZNëu"g?yqxB?€˜82°Þ-?h'h.Oç$?ˆÔïî3?r–I†w?ïȍyí?f/ï_µyt?(êLçp±S?!Âöùç?zññs±ð?eÞ¿zÁ®AGN3FGL J1209.4+4119@bñàm"@RXfÀ(yœÀ:×YîˆßÀ;ÖEßÞ"¿÷ÁèW´›@SxW)²?ÿ2Àœ'È¿èѸ®Õ"¿á
+¥Rèä¿Ã7DԊB¿ãÏK4åCAGNbll?ïütYiB?6Ïo‰c¸*?!š‡M…s?sÔ̦Âú?3Öײc4?2"·ýA?ï»YbÐba?‡Ö}ñ4š˜?n™‡±ªÔu?'íG¡ƒa?sŠÁ¹.?u —+€Ž?Tn—7?yl¨iÔü?v´GÀ=N?k½–…´Q?ƒþøäû?q߅ú¾í"?ïß8hb{1?j´ëŠ>ñ?£ÄCHÉ?"Óñù2 Ô?p<ÛÈ|'?j]#	€?ïþts*«?&ˆGë@WÔ?t¸¹Éñ?ÖëÓ³³k?$Þ`)¢ê2?!Õs'[g?ïçÈ¡ÍxL?eTQ7>~k?T¡ÈuýÝ?RXA¦»°Ž?[Ì󲘄Î?^Xú˜ñ¬?ï»{JñbP?cT­_«Ø?khÖç+•?QV\^J?tï9­a?\ì×öHáŽ?ïú¦*\Ü
?AkÈsÌSt>ü»z_EÇ>þù¾jš?Dy¾IÆ<?AB…Ø€P^AGN3FGL J1209.8+1810@oºèÀHZ@S9Y_í¦aÀ9gšA_EáÀ;¬ìµ `]?Ô¾t~
@ÐXAŠŽå@a>ÀZ"¶¿ÝF\ë¾T¿å¡•¹1±Ë¿çmP@Ê¿ãyU­lÆcAGNfsrq?ïúL熮Ó?BÂÄñRÎû?;+=镬?=¶ïJ+?2mƒÕD`?1£}¾Õ?ᅭu´P?}÷`Žä?ku°†E)?pu7á¬üx?r´Š˜A"?tZ^+•–;?ï8I‹Að™?…ŒÞΖ¡N?…Fî@é>?x%ieY)?Œ§ˆ=ÓTŽ?{®ÀñÄøF?ï̦…Õo?v4X‰pb?Pt²ÍþÁ3?PiŸé°V?uS<%?usÆ>œ×"?ïý©¼&Œ\?4tN·Íï?(ÖG¯£"?3‰ÊÕ?ñ±³?¼Tõ>?ïæzOýCb?h¢LæDæ?UU¶Õµ?T<[kÜ«?]¶E¬"u?bpÈ 1ý?漏ψ‹L?s«KÐêd÷?u},N†+™?k¡}Aââ?w»kð£Ê€?jsÚ4?Ö?ï÷µ{:'?N^«Œç1?1ú‹Ž&CG?%b‡J?H.lã¾$[?Lš"%HtAGN3FGL J1212.2-6251@r§µŸôým¿Ôl(€/mßÀ7ʇJâ|aÀ9Äcôœ¯?ÀùÉ«ÁJŸ@Þao@ç v3¿àU¬9¯N7¿çF& 'Ó.¿é8¡Nè¿ãœ€w_OTHERspp?¡™è˜âñ?¥el¼!öù?ÇAJkš>?ɶYeö?éä3ñ?ËDbîÀE3?¿!ې¹?ÁôW0ϑß?·'ý(›?µ[)ÀY?é+Ë>#Ê?Æ°ý¨%½?»;–•>|N?¤SZi.Í?Ôµ¶tŠ…?¹¥‹ü^F?â72Rë4?¹ç¦
î±?Ãú§Ç?¾N»
=׸?ÞRv¾z?ˆw]¬ýF?ê²NåÒh~?¿,çV¢	?"ДUؑ¶?˜a%‹ŠD?Áëx<F
?ȸ!#çï?êޝY9#¯?ɚÁ'9Á?ΓèÖ{Å?ÐÓ+zpù?¹òPæ~?­1²²',?å»ß-'M?ÏË×øW©?À®÷LY?©X…?T¸?ÒwQŠ·)?³§1ÿùÂF?☵gŽ&?³4&m¸?ƚ¬B'uU?ÀüàE¥{¥?Šó!0w³?z«XÛ¦ÀÝ?éíˆjáäü?Á:>ˆYˆæOTHER3FGL J1212.6+5135@aÍ߆ã´@PM`#UÀ:'tVéñ¡À<ù7Žâ†¿¨n<OÕä@Å´'Œ¶@‡gÿ˜§¿è–'þõ¿¿Ú€]Q®5¿æÍNî-MI¿ã:©xx¦tAGNbll?ïñ˜é<ç^?]n¸cl¦?TÝ®ZgÓ?[9À©õz ??ÁýÊÓ ¡?7ɋ¥zàò?ï™KØ	…ª?†òðßúÆ?ucKõ•"?rþ01•^?}÷½?'£cã¥d}?îòêbKç?‹Û;uX?'Û[3l?…½H/¡Š?°·û?x¬èŸqåí?ïNO
¯@?ˆ8À$˜?ƒ2¶>ø"¨?xøØݾïå?‰9†O'¡?' @\{}è?ïü‹/ôd?8ô¡_3?0ò¦è	s?5†Æ]?&þYö?,8T?ïßDÝïMÅ?i–0OFmÜ?^'‡xñ´?\ë±NJ•?ar^wõ§?a+ð ë0?ïŠ9³f/›?sƒ¶v¨·œ?§\bSî?n¶ÞÇø±ë?{;Ê\3Jn?c¬ ©[Ã?ïà@¾ ž?apZL¦ó‡?`5³º…ä?JëƒÏLÜ$?_‰7îL-?[w"âû|ÖAGN3FGL J1213.1-2619@rE̟¶M@Aád ;ëÀ:1û9ÈÀ;¢þ‡Yûõ¿ì‹›óÄ{@`•™¯¾õ?þ.Ԟþ2u¿ÞµÁ"I«ñ¿ê¢%ùR«¿Ò‡¥; ?‡ÜèñÜAGNbll?ï÷ôNY?H9×ãÆ1/?썫´?C¶¸;Œ?M²#ûž ±?Gmn®¨ ?ï¸ÎxH'?€º±V£Ÿˆ?mÈQ(Y?p'ù&óæ?t´šòw:Ñ?x¦>ôT¡¨?︡Ä?‰úš"Ô- ?"j$]˜¼™?xGË%ľî?"óÙªK…Ÿ?ƒåcü®?ï¥+ˆ|œ?~c
K, 2?ÅtSM!'?"	ß_‰?†'"P£©?~Q
yq?ïü
ëê¹?1'¶>"?':â¶?ã<õ÷?8h™v>}?0jgšaÖ?ïä¡ÐIÙé?eE˒˜O?We¾uLJ?RÄ©­Úä~?_V Ð½ˆ?^…îLۚ?ïŒ:Ù
Ö?r½¶Çîô?vhüí ²¶?d¦h¥Ö÷È?¼üûõ
?lLò$‰Çö?ïñ8XzÚ+?P€Ë+G	>ú³+
ˆì>ù™‡lw¢?]$ƒ%Š»?PmâÊM¶(AGN3FGL J1213.7+1306@pί€Uûµ@R[¢Àh¡À9¦¦J'RÀ;ÁžÊ[…?îâä]&£@r°¹Æµ±@([À6ã¿ãœýd¢Êx¿åݙíÁ'í¿ëÉV~D‡¿ï÷c"ã©AGNfsrq?ì~Îs"ËÆ?²~:}b‹?¶3ÑÆo?±2²ö0?—YÊ?·w'?'"P¯oð?Òå0â²"Ž?ÐRü$0êa?ãP'ò|ù?ÐBvvm´R?¹êx]£þ?·p×ÑG6Ê?é':.œm?®™'*†Ó?¿ç:™%wÖ?§È÷-E?´óó®î(?DÚÎ&Æ?ʕí@ú_ò?´'='³
I?çÁŒ-åk?¸ Ë >'È?©ˆ#Ɋ'?¡:a1é?íèktÿA¥?§ôÚ¬
>Û?ªñíëè>?¥
àêQ?Šk	‰!Ä?"áÆ"d?áõ@~fý?͉Œ¨'Ñ?×䫉8Öê?ËN—ÎÏl ?°ÃQ]ߑó?«æLß-Ö?ìÀ/ðU	"?¢6Xóp²?°çêy'?›º&¦È?¢-+át?•ú=?âäSÛ¹ ?±~¨
Ùe?Øtºa»0î?±ÍCª6»L?œ)Þi»4?•]—"fcMIXED3FGL J1214.0-6236@rªI`0Â@¿ª×'?á
À7Öå•ñnmÀ9Õܨ#$?÷Nu»€Ê@>:\È-?þ¿Ü™žw$¿º}bVa`˜¿ãÜ[ýVØ¿å%±Ím¿ézØC""OTHERspp?h!YЮ"5?`œ#‰Šic?ƱvÒf·?ÅÂ'åÀc?êe²H´q.?ÅÝb'o©†?ãIxà_¨?šöúÿ­M??Ȟ!Ïĵ?»ÞÄúy?é`êfÔ^?¾Új§
<ç?¬¡`O…€0?™ß™Dþ¸?Ña
¤¶á²?·M,· ƨ?å…c(ºD?·F0У?«[–K'èõ?¦°`­Û>+?À~j'ïx?¬Ñ8Ž´0?êC§¬Å"?µ€H	Úò?g…Hp?e2,®"u?È!KÒïÚ!?Äò±±›÷?éà'†Í?Å~V/"?¡kŠs©…?©–L<?Ðö¦a
·?½h.I‹Ü?æmôVBp­?‹8Wà?¶Pkñ¶SH?£&ÄíGÚ?Ñ N¡\?³ÚÍÿBcÿ?ä¥Ëx†E÷?´KýÄy\±?«˜,L³8±?§Î-
T?ÆF;uG;?¦Í¯µ_©Ñ?è´îs)‡'?²ÓkøaÓOTHER3FGL J1215.0+5002@a,ô!-w@Pƒ¾`"‡À9þ1Ýȝ"À;ÔÇýZ3R?Ô¶G5"ØS@RÙþ
·y?þ¶
 r~?ïIJá$É¿çoO ž¿ÁTªYãÔ¯¿åѱ'­AGNbll?ïíÞÐZuí?_meà¹ÑŽ?2î:YSX?0où§Š!?_†ÐßÚ?]§GM¤³?ï3Ö·f÷?"ûŽ•ÕJè?‹_ogœx?ŒÛ'Ìñ–Î?‡ªâÌ{^¿?ŠkuÛ(¤?ïñ	m%?‡Áø>‡Óˆ?"0QLêç"?rX¤Ýs¦Ô?"é¶2C®‡?ƒˆ˜ɞ÷?ímªÌX?ªR¬3õÜÙ?"¶bØ0eö?'—Ó4´¬^?®Ê!Ðùñã?§‡$£­¬'?ïú¹Ç/?C
äÄ=Ä?"ôµêke?!L2þmûN?C;êa2m.?@¼_5/?›?ïº3ÖØOž?vΉ
N­?st÷…&Ï?n @èS—&?nâ9ÿ&҂?iݺE4·H?ï‰É~Cí?tõpÎߊ?vì©ÇE«?`Ì°ØZ‹›?'jòë"?qž¬H]êÔ?ïV¶§éµÞ?†$Wv%_?…õ¤a'¥?u:ª´/?"Ð`a0õÖ?€7Ô¿tÉzAGN3FGL J1215.1+1658@pW"_ôö@S4z?̞ªÀ9´`ÎvñÀ;Àh‹Ô¡?èRßúÅ:@Gt.©6@‡¼Ÿ®·¿Ð1Ƽ›¿å¹6²Ää¿é÷ÏM
WŠ¿äœGãˆ?AGNfsrq?Ø¥í?†öSÿ'?…¼PëºT£?†=s?TéÈêAª?P=Jà…}Ü?î×ÿe¦M?­"4	ú?"eklÁ'?¦Ê¡Ò·Ã1?šþák¤?˜d»J×/J?îzQàrq?"(҇ ñ?š¡ˆÓ-ó?µê½`Ž¯?–;%Žè?'æ#¦Éf?ê~#
_ï?³U"¸«¼?ÀVF`GÐ?²ô½%öñ?®]è°±wØ?¤5SÈÕ?ïë*{²0?b¥K'w"?`ú¸bÞ¾?af7Ö©Å	?>Ö`;¦?5½‡ó¿¤?Õ;A†?•?˜}W?|…8ÆþH?¼Øº¡?u±ÝNwvÍ?ø#r_ë»?ï>î"a-?† sd'?Œµ¢»™Œ?'NóN‡õ?ƒŽ¸ÙgC?t
Žv•P'?î‰$‰w7š?"*q6±¿l?¡QHtg®?‹ññ}
ûI?ˆq»àꆴ?"ê5ÊYƒAGN3FGL J1217.8+3007@g›îàóË>@TƒDàá6À7i1"·ºíÀ:®•­¤é?å^·üŽ¹õ@Qˆ®d×Æ?ÿ—v~·k¿àÉø՜޿àDOÌಢ¿ßÃ`uiA@¿áùùšzAGNbll?ïùpЈÕ7?P\Βí©?0X1¼¡Y?/ËhïuZe?B¥žUÒ?N×ÿ‡8ú?ïí©¢az?®™–©)®?p
ÜÙי§?q–wD<í?›žÓ˜­†B?®6Ò2Gø?îÝñ?üLö?™ábÏd?ƒ»>dQ©º?†^¥Í‰S?šd8ÇnTw?"æì-œ7²?îª2..L?šU";sº?k¡~jÒ?n¿'@J?£¢Å9Ë÷¼?š=GÌ+îð?ïý£¶UM?,+"Ò§Ÿ? ŒUäÖwÃ?O§rŒÖ—?%AàÇË£ç?&ý·:¹÷?ïÄ"Ò?ŠLaTÁ?[Հ¶&j?\˜"Äš9­?vù6Òïåw?‰%ôŽ¹•?ï^Ko•?Œޘ<§o?z
ïr>5ñ?yÈ*®ƒÑP?‹rõ]=1Š?ˆxÛ@Õs•?ï™ìÚ֝(?|/¨@xh?]ýڗ(æª?S•â¶‰5"?…Å
ê
Y?{ê-#…[kAGN3FGL J1218.0-0029@qÖÿâ£Ï@N¢ŸÒ˜¿À9|Æ@Á'/À;sþ¨+¡?àÁ Á"—@··M^­Š@]a#Ü¿äóa£ý‡¿åjÊ!)xþ¿êGDŒ™Mf¿ÑºO­ÎkAGNbll?ïó¼oä?W›`\~¼?O²Ën°™?Q¸˜®QR~?A].{oqí?BT3¬u¤ ?ï¯Ä#¹?‰®ÿ"?rI-îoq?ƒ"ÿ¶àÑ?uÔ_f勹?yWpôn°B?ï˜(]õ²?‡è<Èeèp?‡¾¤)»FZ?}"Œ»ûôL?'m¨Ý«Ø'?€'aOý?îò\:µÕÝ?"Ñ
d«ýÕ?we˅ªÇe?|1³¶x?›ÛÇ*¦'?'ª~sll?ïûÛ$PB?>²–@›D?5+ô¯"ō?6Ó²BÃôx?'õÖt]Ø%?)4:¢nу?ïå/`Qq?ey\plò@?XÎðë{î?W›(‡­Ó?\ÒèÍÔ?\dN0?ï–-¸í>T?yA²û
®?yˆ)€"&s?u9cøo·L?{`ùÿݳ¶?gåè­ì?ïÌ:ç:>ô?q=²°b?Z£Ç›Žª?UHÎŇHˆ?s9šeÿ[¾?m"'lù€AGN3FGL J1218.4-0121@qà|`Ÿ@N5æ`ɊÀ9hq¡›À;`qå©é?Þ0$ðˆ@RìéLà-@Á?zê,¿Úà'yõíá¿áVzšÖ»¿æùïã&¿Ö·µœb)sAGNbll?ï³ðق£ð?'ù¿bðª?}+ŝÜÞä?'+àÿ?Øá?a·›e^B?b§µ×ãåA?ï{!Gèã?'êÂÑØA£?~Z-eñMï?…‡ø[ÆÐ?'
—Vrü@?Š.—|ÆÓ?í½øÆzÎ?ž 0¯ÇĪ? ª_ê•Bn?'^'?«~®?£" ‡KB±?"ûág'}ñ?ì]i%™¨Ä?§sI1xþ,? $rðËJ:?›'¯øÍÿ?µ}[;@?¤J9‹Ç1?ï¥+$¾GÆ?¶Ñ‡…e"?… Ðû
[?¶Õ¿º•'¤?IR £Bæü?I9ÖΠçã?ïÔى@(?v÷½¤¡à?dç³&ä=}?n¹o'v*Å?gs(#5?jGÉi'MW?ï  ©Ã³I?Œ
fÕSz?·ÅâIw?ƒQBÿ`H?Š@°9R¹?€uò7LíÎ?ïÉbpHÏ?†ˆkEn?'ñ㒣š?rQHÒ>Â?'­áéÙ;à?'‡b/÷9AGN3FGL J1218.5+6912@_Ïÿ`Ï‰@GÑN¿ÓÀÀ:O…¯
À<îøp¿†¿e»_p_¯Ú@¡P&l@&îÿ|¢h¿ê³~ÁT¿çÚ:Þo®Ü¿ïª¦!ÅÖ¿ïí7©¬–AGNbcu?ì'F•­?Ïkü ÈÁ?»[ë"Î6.?ÏnófG<?9䤦?çS??N1Ȧ ?îkÉ+{u?¦$?`¤@Î?Ý{+ŸŠ? Å:ˆXj?"©¼)û÷¿?–—÷¶ù±?íàÙÁý¼?™Dí«û­?£å²‡Ëø?"›€xÂM?œ2Œ°°•?Š{]np $?êÊ_úçgX?µ¦QIÐ?ÀD7wªJ?´§írÉF?¢G‹xÒKR?wÝv'â?åDæs‰\?Ý•h©Ùû?Õs}°ÚÓÌ?Ýg5΢?%«=ª)‡Ð?.# ì^¸r?}*?Š§Ãñ	¯?}ø]B%{?ƒÂýn<â÷?u¿ŸÃÎ?{PpÇnj?î¿ëód?Ä˜3rï?šâÛÝÝ?§×_{?Š?ƒ|
Y?z˜U¨‰?ïcO¨(º?ƒÂ¼d41?‹Z£4"f?}n|]Nù?w£-^`r+?uÓéŸ÷AGN3FGL J1218.8-4827@r•øŸƒ¾f@,•"d~À9—æuë>¨À;…ª8MNg?ÃA¡b2Fœ@ÅUmðžc@°zÿzŸ¿á»Â/Ý4Æ¿âR1ÙR¿ã-1ò&µ¿ïäšZAGNbcu?í*Ì?²ÔÕûaÅ?´epÑv_?°òydø¢?ŒÌ·Ò_uì?'UâtN½p?é?zÚØ?æçüº6ƒ?¸Ót'#K?°I&Û#?½0´­
('?¼·s#xx?êë|îÆ¥?®._w)?Àèô±å?¨¢0'«$?¬b—'q?"ÁêMz?ès#$¥Ú?°ntÙò?»F?Kç¬?ª°g39e?À§pSÇtÁ?¥]ë_ãT?ïg=?À?˜žJE'òâ?˜²¢²?—£Å¬À?nKˆ_ü''?k¹E—÷öw?íÜ®ÅáÝ;?«ƒH»Å+? íð*l]?˜ä¾äŠaK?¢ %µ'[è?£Îíøç>?íQÁ´üݝ? #<²BDå?¯I1¥©G?›Ù1܇Z?—5fê³Ü?ƒšŒI(·?í¶(¬­®¶?"Š6){²%? j­>"M—?‹'Ää9?¤2Çó1+?oØIAGN3FGL J1219.7-0314@qù€#¦Î@MWý`OÀ9ÆÀâ³¾ßÀ;–ÿ³©æ?䓒T3'†@Á!ý*ãƒ@Ÿ§Ð"¿Öyw8':¿ÞU#ÁXØè¿à'Ž:ô¿âߙ
AGNbll?ï°2EU'W?7â-%äÖ?p_(ŒÂ—Ô?kÅʃ«‹?w‡´èöM?xۋ;
ñP?înPOE/?§Û_æß6v?Â€ŠØJT?¡‹k´}!s?"su•ۍ?™Â °Öuc?î"]"£v›?–±è¿,?•=_VÞ¦B?ƒæ7Ò¶8?£;~&é§8?ñ¹›`¦Û?èØwÚù?¯·}É22?¼Í=†¯mR?®cW\@?¼o	–4gï?£¬˜ÛËƧ?ïÕòîIŸ0? I5xé¾?R&Åïgq?QùÙìŒ-?p…ÿ)´õ? }GÇVü?ï›ñòîº?‰hK"=?{¨ÊªÊû?€ïÐB….%?v^<.ƒñ?zãNmÈÇ?ïE ÚÚÆN?ƒãB>šÃ±?ƒÊfÒÝ1?vpŒ™wÕ?Šíbk…[?~}ÓþŒèÒ?íG°ž'?•žnv(œ?¬Æ°šeg%?'
LO×K?|‹|ó{?†õî",ŸñAGN3FGL J1220.2+3434@d^Õ•:@Sÿí ‹]À9à5"FK>À;éC¡É¿êÕõ7zÄ@`<O´X@oÿl\J¿áò¼:ƒ^š¿áËcÁ¤\¿äŠÝcÈÒA¿æàBÙL´AGNbll?ïâ%hç—v?gk›Ø®Å_?Xñè-…6?\H*ò`ò?aa¢ÃÍq?[öŽäø#P?î·¶'œ?°£®üm¾?{Ü}º+
?€
Ù"ô¥?¡ƒ553A?°p´@`ƒ©?îËm/i‹E?«%Òl?‰'hXKI?z²÷ä-›?™ÉNÜ꣹?ŠÒ$"׆2?ï6I[ÏÅ·?úa_}…?{–ÔŽ©MÜ?x"±'CE
?'Qcd×°?ŒXü>¬?ïõi
µ 5?S°sIUµ?A}P+=–?FÞ£'Wu?HÞ®}'²D?Fè²Ý3Ù¹?ﯠ.^7C?×;ª²?b¾éÔ×G¤?b™Š
F‰3?~ÐsÐ{:Û?zÕø??ï|'`
ª?€¯Ä'žt?{t"Ú@bý?qœ¬`S!o?ƒ!ej¼Ü?{¤ÀMû?ïàã`ž6ž?gyÞވ92?L®;š‰ž'?EöTÒ¿Y?gñn¥3³?f3cØÖµAGN3FGL J1220.2+7105@_¢ïÝëÙ@Fè|à%o%À9Œõ#-+²À<|Ñâ¶C?Ò@XXå@ {KÆÓ@²¾ aŸW¿äII0[Ï¿åÁc"&¿ê"x×Æꤿè[ki;¥AGNfsrq?ïýdͽ–,?+•Å¯|"E?%î³õʈf?"#ë7{ ?#Äpe™‰5?§f'FÏ?ï¤OÙÃ;?†.›ÈÀÜ?t¾'lĺ?r»í׶l-?yÕTˆ%ÿr?€Ã(¶èìá?ïMZ_X;g?Æ‰qs*?'á
¹ñ?x€F®?Š‹‡Sd?vÈØVÜÆ@?ï¸éëìw¸?ÄþµÇ´?i=ÿG¦æ?dµî´µ.?wk?؎?CÞ%3œ?ïû
Útf?z¨M#šÊ?AV­¾kŸ?z¨¾õþ…;?ô\wН?
¸îJÌè?ïá'OÚD?gëÙÁµ<?[ô‰|²'?Tʦ¬ÙU?`ÿd,
P?b	dzm?ïŸ*¤]0Ì?|Š²rñ˝?uràñ¿™â?sÛ¤ӔÝ?z÷ÌûÔËÂ?t+oõÒCË?ïõØÆønÞ?X7	˜æY{?@ I[?4'5H5Ô?H
ÂØ?Z?U"®+J©@AGN3FGL J1221.3+3010@gKØ't@T¯ &5À7É©f–7À:ˆ'–9?ٌ0¡Ð@Zys3~?úèÀž@G?¦cMû¿Û(ó/sû¿ÎŸ5åÀ¿Ñk…ÎÐK÷AGNbll?ïÌÐã)R?€·Ê&=M?:>ĕø¿?;Šu¡§Y?wó¢ífÆ?96<²úÈ?ï)þr¥þœ?ª¬£Lé)?rÚüå=6å?~›ª'ÅP?–	rjaºÞ?ªLzÎo'Ÿ?ç½
ŠŠ»Ž?´B5
£¸Ÿ?¢ÅÇÉþrT?™©Ä>pÅ?ÌZWã{t?³?È:«rk?êáÜ®8¯k?²¦u¦"»?yö‰Rk?{Iðp·>m?èØþÖ¬—?²¦—±qƒy?ïㄓfé]?t{!T՗'?;£½8Q×H?A0ŸÑ]R†?iôìF©Î?sG»Rijæ?ï³Ø‰ÚP?'½ióÝ´†?b{	û?ú?l™šeZn?|Ö6'æ@??'
"Û£?é¡þbWI?±!açTº?¢a¥s'Þ¶?—ñ‹#ev?Äãv©Ìäí?¯Ó
ªX!¸?íó<Ž·Ïv?±"¾ç§‡?qVú›'?cˆ.¨®?®¨ÌUm?«?Õj9¶ƒUAGN3FGL J1221.4+2814@i5ÛߏG0@TÑî¿Ñ;ÇÀ7ÍÜcBÅwÀ;#Pg ¡?ëäb''k'@Fö¬o4@@Ñ£@Œb$¿Þ"yt51¿â'î÷øŒ¿àܽýôY{¿åXlR¹‹RAGNbll?ïú®÷µS?DX.°@{­?+''NŸ¸.?)y/"[ËÏ?<Çd»ín?A«Bn6?ïÁª¯Áy?«âL)¾J?t"K'<j¢?'LmŽEJ?—Æ·ÇÈz.?«¿¤MÛ3?ïS÷Ó®	à?‰-0*cWž?|ÄkkZ»?vRÒwÜK?ŒŸÕR?X?…È2M?îá-2y`$?™Ô)ö9%è?}¸"—¸T?{Æ÷h´KÛ?œ"k‡bŠd?˜Ô28x?ïý¾G[3?&;ý\Õ? 8Œ»"SG?ðg÷ÐDÀ?#Þ}Âp'P? ÅáÄçÈÝ?ï©«zl­¨?"çUž"?dW0&…7?m]³ñ¨ß?€Ui¡«Í?"4°]kÆ?ï›)*Š†ñ?|xlèQˆÂ?s*ß	äÒ÷?fËé!$ä?@‹ÄÅp{?y"jmÆÿÇ?ï¹^Rñ"'?tÁÍ?cm?iÍ«'9©?]›Wì9?vjÄ´ò?râxSAGN3FGL J1222.4+0414@q͞?»×²@P…IÿþRÀ8Fˆ'
YÀ;I_ND0±?õ±Óšt¦@ôDÖÙZ@Aâ:È'÷¿åk´¿˜dn¿ê–î¼ê4D¿ìíâtåì?¿ÝÌùˆA­tAGNfsrq?ïô"²Ñ?`^㪸[?P´—ݐï?_Tß?h
A?8HǕè?;Èîù8O;?ï &ÀÖkÔ?‹ÃgŒÅå?vÎ~¡ÈF"?"™Æ€¦…E?y!­û?~GºZ­–>?î?,³Î?—c¢8dû?"
¦qû7?Ž1Kû¡¹ˆ?™øÄä¹?'x ¾óc?îcÏNÌÀ?£wŒ]ÙÀt?"¿ßVü¶Ö?šŒNdš'?žÆ6Ôª/?žBì–Ia?ïú\™+?WZ<-Kk?:Mq\5Ƒ??8?º_?2ђHe%ÿ?UâÓM0;²?ïÞí%)Qª?oºZiîÄ?`r?ai?`êC9b?ah"Œl9?eüPaäñ?îû¼;¨?Ç!G¦?1Q•tv?…)7a	?'_óêú´?‡VeÝík?隣AMtŸ?~¿õˆ¶¨?x²ò2óTn?pzýíl,·?stmõ?vUieŠ£{AGN3FGL J1222.7+8041@_rÞCí–@B,Ò?ÓT¦À9+ªëÑtÒÀ;Ç«ZŒ='?×ي)(H@áuÁ"I¬@HÿÚÁ,¿à½'i›ò¿æÔ/[¿áå(­b3¿ê¸ƒÑJ#ÔAGNbll?ïö¯ðP¾?J¡Ÿô´¥?H¶ÝÔ׊p?EŸà°	G"?9ÃGOY"?2ɖh¨?î÷Òù¦cp?˜íáøÿ?'=—#îS?Šìanƒ6?ØÆ]ÐsS?"Bt¢Fð?î÷Äb&r?0Â{Ì:g?'–
¯&Yí?‡4¨êtœm?ŽâÌ
k?Â?nªÚ>q?î;ðå—O?œƒÆ@
-²?"ñÚUÿïm?‡ÔBOl?¡Èx '\?˜ 
‹Š¶s?ïûj•'͂?8	•.Ê{?:¯h&©C?4^/?Cœ?#ø¢Nqˆ?š‰'rÚ?ïx™÷Ÿ?'—‰öàÞ?yãUðåjY?wÆ-'Å?w`b\ëº5?yôY~¹?ïyø:Jþ?'M›eŠ•?ƒQ :VjÖ?}ì–,Ûâá?|`¢{™?3?rŽÝ£€Ã?ï¡ÄS®?y;@§ËŖ?x'k?g†Ï$æø?w-hÊ?tQÙâ@ÍAGN3FGL J1223.3-3028@r|˟ÛÒú@@‰`fr%À:vŽŒ]"À;¼ól|*?Âv¥´ì@
¼Œã¨±?þ/ƒáK‰ì¿ãšOˆ¿åüqЧͺ¿Ü
«±Ò©¿ÉW̵AGNbcu?ïë(¤}E?`o³U{1M?,OJ'i€¨?(kg†¤Î?cì™ÙHô?_JÅ4uÓ?—ÇKG?†à—§H{;?r̕9΅ò?pÉiGñ¡
?{ÜÈnÎ}?'óá?ö½?î⇦Ÿ]ö?ˆ…¨¬ú"?"»ÿà ?p9ýPo?™Qƒ#-8?"É«ÍQ@µ?ïšÜ9?'Uo"k"?déN,Ǫí?p%4×rú?›Ï•Ö Èþ?'T4Z"ï?ïøÂ:ôÒ?FÑøý×_k?!kTâÞª?¾J-o÷X?HœAê©Jk?E2º# ØÛ?ïݑ0!?mK96ôÞ
?\˜"¼'—ø?U°ÆYߦ	?d"âRMY?g˜±çÂ?ï{¢J¹N?t³d-=†6?w7žúñì?[$éÄTXG?…{ñr<–?qI§"à'?ïÍÈq$Û?k
i¿aÊ?TR¤:ýïê?PxT¢&t?t說?hªiÛCè¢AGN3FGL J1224.5+4957@`¼ÿÚ@S@P¥é`êMÀ:=އà4À;á¼é)ú¥¿Â¥ô*]³@L¤sgUÐ@´¶ŸcÝö¿âµý¨ëNÌ¿ë'Éùkø¿Ó7"E5­ü¿ëôHÖAGNfsrq?ï÷—@n¹?P;Ú4¤pÕ?6¸áª†`Ç?5
 -…¿à?FFŽ­Äp?J7À sL6?ï~鎓E?‰Ì±N5$÷?~1ßðÆÊ?{}…Ôx7S?<^'×K?ƒ7I®ü؅?î¨ÀàÒµ'?±+<¶íý?Xpž<…?}§-#wE?šÒ‹uM?‰†šÓ[à?ï ÝôEe?ipQ¹À‡?y¾r³{?uªUƒw?•t¤Ë.š¦?‹rbIÖu´?ïùÉFÒÄ«?Džú¸áÄ?4ï—ç«?2ÌF8JSž?<ÆÃÈÇÚQ?<È'b،°?ïÖ*ë!\Ø?kâü'#?eèÏJ5?a3dzùý?cìE¥«?`
\ªÆØ?ïF¹ƒØ×?›Ls_kö?†¦d¬Ò?uRÜ»U?ˆK­>­‰?y³šv¹DÛ?ïÏ~¤˜Ñ?j¿Ð'ºV?dHhAçdÖ?Uñ8ʞ_¬?l9	ÚFúe?e—ph(¤AGN3FGL J1224.5+2436@m@ôŸM¡@Tܸ¿ÏŽHÀ9†_:øúRÀ;ˆ›†Ù£?μÛÙì+H@𪮔Óa?þ0é
ìî¿éŒT¼ð¶·¿Õ0yשÁý¿ÔûòÇ)¿ãπل@AAGNbll?ïóˆÿ©ª?V-¤˜‰¥?@-k´ȏ?7yÜR?1ˆ?P×Jü;ó÷?SÕ#¯CçA?îlå2&Ì?´å}ñ?=Œá!
?€Z¿ÂÛÐ?¤âL`·Âþ?´Í®.öo?ïÃî¿
?›çö ?-HÀ³}?rŒ9Ñ1\V?"ÐÝÚd…©?"T#ÿÊ·?îXÚépO?"oMeqS?é¦×'¤?"ÎçcŽá(?¢bܝi Å?'ºg
i?ïû´mt;€?:_Îï´¨?.žÀEPI?$ÒýÂÓÄ¢?3
6Y±û?6dÓu	m?ïÒé¤ýY?šÈ<[7û?n"â}¿šž?u30íÕNZ?"&LíïC?™mO¹¦ªN?ï~ÜÑ •?….jP?t»åÈ]?fä@ՇÚH?…êØÙþí?"'kLÕÏ?ï~6Üàì?u"®¹Ýúü?H™«q
?dêý¥·Óú?€å¤"64Š?qoªh7±AGN3FGL J1224.6+4332@anýæOU@R-‹àôÀ9´Rb£cGÀ;ÿžÁ÷†µ¿àºñQ!ÁØ@­á­.¡Ô@]  Ö¿æh¨µì6¿è õ(¿Ž¿æW|ûBð¿ïÿ⾦™\AGNbll?ïò!U:D?_I'Êê]Ð?8Õæ^hË?74çÎáR?U¶Ø&¸ø?].Ë	z?îƾxK@E?¢¾ïH£?•±®–ß]§?š˜É6Šï?'v'W!"½?'D*œù¯á?ïuVyÄ?Š5ö!¨óß?ú×M?~U"'èZ?´®­Xç?ƒ0v7JF?îL㵓í€?£FðŠ"7d? m\™›ão?ž"'"—?•ˆÐ!)Á&?"*Þ=?ïøä7ñ?IfïïÚÍz?1a'²$V?1þ&ëôŽN?C¼ö‹ë} ?E7F@õ|?ï­¿q3c?…õ¢ˆM
?v™0#.,?}ýÆۗN?räp0UdŒ?u¯Ü ƒ.z?ïRVÝînn?'"†ÚK!Ô?‰ې-6?xéKŸñæw?'j6¬ó¿.?z*–§Wås?ïÎX¼jæ?rÿsddý?g²ô'ø9?dŒpÕïÐ?iôO#ÿæŒ?k|+"—GùAGN3FGL J1224.6-8312@ráoŸËÀ4a¦¹Ù«À9zeÜÓ«
À;{ ù	kº?¹3ݕ+}@#ÏÃøõ@Ž_?«'"¿ä‰'å´g¿êj\´Ù2ƒ¿ãü¶Ôâm¿í|3FUAGNbcu?ïç$x¢?‹€˜?7©?vðQoÕ?vÞ
d‰å?"ŽÖG?"ç™ ?í«è&֔³?±ºDFòPí?—•twÊ\?"Ȑ~Èû?©vÃV±†ƒ?­ßcß?Ä{?ëÊJX‹(à?§/X:Ý)D?²Ö÷¿ôà? Î~üÕì?­­jõ«ä?—ø0•Ùw~?êìKV¯S?¦©îÊzAx?h æAŠ?‹`Æ!3—·?À¡¾¡eëÂ?¥]W»Q?ïŸ#ÑM?«;¶ÿóO?}ÝÄJ֔?«5Tc™'e?r'ifüYq?n·^	ƒ^?ï9x¥
?˜G®
›©Q?€ài+y•Â?€:µ(};?`É>k§?"8Ç­å<A?íýø¢NÛ?—òÆ­Ë;?¤­"™z=r?'Žñ¦Ê$i?–榆Ÿ¾b?…'Å…~Ü3?†Wâ?ˆ7ʚä	?‡À‰â0P?qê~2½Ç? WÛÝVŸÙ?…è°@¼&AGN3FGL J1224.9+2122@oáç_ö	Ý@TjV ŘÀ5û‰SÑ8lÀ:e~ƒ"×?ù»]¹™";@#šŽSz@ñcá¦Î‹¿á"ìÂû+Ÿ¿åOA
çIP¿äÔ]X†åô¿çH%p|ê·AGNFSRQ?ïÜD'½B§?pû‹ä;´¥?OªS®Ô?R»$(\%?kÐØ"ªõ™?o…ŸŸi¨•?ïUtƒµ­?§ÚWsRŠ?eãrñD?m$Ì®'ü§?'•ú¶ÖF?§\KfŠ?íG
"'¹j?¨²¤çÝH?šaʐÖ~1?–`º//PL?®^BoUC?¢'?r ï?ïþê˜S5?::}z5B…>µ/ŒœF">ãË;è7?!,™»"?:5葭XL?ïí%N\ô?q	ªêÍp?OwV'.R?aðH8:?Uù¸Cý?dT™rŸà&?ïØw5Ÿ&Õ?"Œ/óh?Râ&·]¨?R¶Øš'?n¿íä"?ƒZ>0"¡?í‹[~^ˆT?£mú2¨Æ?–c»bØl‡?'')L›?¬jjcw? AÖC€ù´?ïÿÛ.(K=?lmA½>ŽNsêîUü>£Ó'!ŠÖ>ò,W[½õL?jzáu:.AGN3FGL J1225.7-7314@rÐÛ«–òÀ$íG¾Ûr'À9á¢!þW‰À;s`c'¿ò©0
3à'@>}[ËWØ@y¬ÿ§ël?çöE€‰q¿ìãrÜÁ¿Àvö%$–|¿çã•&ÔfZAGNbcu?î2¨ŠkK?­~ª-z1€?t<¥ºÉ›é?x놺±y°?ªMë¶=X?¬:2>·7õ?íëóŒ»K?´FùfB[?†"Ô±õ:g?‹˜Ãéuæ?«›'òa?±¿³e›ÛÖ?íÉɶæ?¡Š4úB,Ê?›¯42"I?‰-ކ?±ä¬5ª;? þª»6?í§lÐêX?§íUšÆß?N.Ôù}@?Z¾f%?²ˆBÖ<­È?§Ûå
sK ?ï1K…4?
¼¥9\?]C??eš?\"£sR¬?ŒECÜÏ?OÁ·¯?ïOM1ȋ?(þœ•±ß?pôy""¡¤?sƒ~øÇê?'Ù@:½)?™z1?*G?îÿÎ(%?ˆ°L+ö«?‡¯½Ã%¡S?w¹î8+dc?".]ùiê©?"PkëôúÐ?ïuQ*6¿?'Z'rF*?7$ô_Ln[?2à›
©
º?ùFð'É?'B&¾¢;ûAGN3FGL J1226.8+0638@qÝõ€í @Q,ڀ¶–À:ámmÁ¤À;·ÉjA½:¿ÔôU–¤6@
‹w+/®™?ù>ÎÇÏ¿í··pˆíê¿ßø…Š…Q?ʦ`;ÿàu¿ÕS{ìÏ:AGNbll?ïì›ßšø?i::°ür?93 f´Ò?C×rˆTÃ?`AÙÕ!¿?gڍô'šæ?ï«Ä.m¦¢?'Õ{	õþ?r¡Rs°s?t ²†P@?w|֎V¢?{(DÌF—Ï?î{zF}Ù?•ôý?ÎÜ?‡´ücÑ&?€w.o0
?¢[[Ë!?•YE©rùž?ï Ï"•?––[Î<K{?OuÖ=~|?[Ol˗"ø?š÷'oÅ?–p+î»å?ï÷~EoÅ?Sê0áxn9?&Å6Zûé6?')òÿ5l:?LUœ/!
È?Rún;ad?ïå1¯Çб?g°f ·œ?ZFˆoûY?[mãRï=?[V¸£?[=ä9Ím?ï0'¡Ar?ˆO"±¶•?€Õ‡\†bã?y	ß/+â?''ª@F?…ØFhõ+?ï̕"-¨?pϊ–˜E?Qa°L£§?P€Üù[œ?u\Å>=Fj?m9È'ëd9AGN3FGL J1226.9-1329@r]®@…+N@Hxwò
ÏÀ9.x,a‡ÚÀ;R½¿Ïæ?îƒÝy\&5@KŠó8œT?ÿ¹V  žñ¿ïþÞY‰€"?ïèÏ;*è%¿á"30¦]¿åY¬µç´AGNbll?ï¾+T ö?w<{öakä?wZÿˆ"l<?rSÕ¥C‡ó?c¬lõÁ¢?^Ñ;­'Yj?æZ0/7?Êí@]›Å!?͚ÔÍLN?ÈPL‰›b?±øÔí¡'\?±Á<	(oK?í·õÉ+"¾?ž[íüI:?¥<šŒŸn?—i&¶ØV´?žˆ¿—›m?R3ô§œ?ܚ
ÛÙ¸¡?ÅòŽUÝq?àZHlÅ?Æü%ÞiŠç?¥‹"Qq^R?¥X‰Þ)…N?ïâÿñ?gF'î}?eu•äôWö?a¼K䜯ž?QÕߖŽ,?M!}	næê?ìfAêþ]‹?¼³òuÓÁ´?¶ÈÜA"Ï?¹§Ý!ž5?›0Ÿ//Ãg?š|Ha(õÿ?îí—#-è­?GúäŽê§?"Ö@>¤>?Š^¦Ùø?Œí¶ª¶h?T"Fí?énÆû/>e?³&úî,ʸ?ÇfîVŠP?²ß®ö;õ¾?–öñ#ôDï?pÁv"ÓMIXED3FGL J1227.9-4854@r¯CÀ~à±@+"É¡Ÿ!™À7蠖ãÜ´À;ϹWf?ø‡¤Ò1æ'@Džïnã8@–5¶ñ¿âZˆKµØa¿äP¡KÐÊ¿çü?^Ã8¿êßÿ_PSRpsr?çÍ€g?ǜùçH_Q?Î<åPHº%?Ç,¯çÊæ)?›ÿ4öNGÙ? I*[í=e?ÏÊBõ¯*a?Çg§™Œƒ‡?á¿+>û›ö?Éüàélô?É9beÈ?Â|Ê£I=-?äû=fÎý:?µî$PæN2?ÐJdsƒ@£?´*ýhÑ?¶ü'þꯠ?¢'ê‹¡Î?ËÂq£ "?³ˆ‡xò¿'?âíÌÞYUö?¼c?*m÷?ȆZâú‹¢?³Fǔȇ??î"R^ݏ?±ZY^¢¾?¤í;30#Ì?°¹/è-Â?mÚJ¼œv?yx»Æ??چ¹Hœ¸?əթ•:9?ÜٜiÌ?ÅÜöõ"ç?ÂÐÚ5ôŒ7?¿º$>"Ðe?긴;å?«ðE7úó?½
5ý¬­a?¨-³.¥Œ?ªk8Ç'ä?™´ú'´?Þ;¨;Œ¸?®ßïmO?څ×MŒÙJ?°äÆÛ\Œ½?½×´(Þg÷?£ ÿŒº#'MIXED3FGL J1228.7+4857@`™¥ 8L@Pî‹î²ÑÀ9èûŒ3€À;©ÏŽH,¿¿Â–Lwg@á©Ë•ë@ë€z8Ö¿äVˆ: ¸1¿äS‰ëY]r¿í94?*jë?Ì9¿ãǪAGNfsrq?ï¸q¿œê?‹n˜H'"7?TGâk2?U=L…Jra?~ÁŽN»—?Š×)ÚàYô?ïÃ[m[p?~:ä}¦ž?k#ö)U?p‰8Úô?páD-ú_½?s'dÈN\]?îߏ1¶±W?"jé0oY`?‹*SߧÐ&?€"(=À»¬?–xïÙUìþ?' ºŸH'?ïÀqÍçn?€Y´Bç'??¸€?¾p?K"¸(´`?~>C/ž4?€L݆‰ï?îʟ•ü?›²¿k¡u?ZÙº{¦ft?s
挷û?¢8Ú¼úr?#ß$µŽ?ïç#š[Wâ?iRAÄX"™?U²3V_+`?Wu~þ~óÀ?\—Ú3á?aî7†$??ï^Ž*Ў"?‰•j¦`(>?pC£Zšü?|Bl·
rÚ?ˆ¤SƒvÚ?"S¥"¶Â?ïøN/ZX?TݟmšŠ?X͏:mM?°`¡¥"?L)ÒµÖ?T5ΎXöÏAGN3FGL J1229.1+0202@r¨@[9â@Pr@#Ü~À6nç=À:Üš\78?ÿ£"¦%@!ñ@­DFV@Zâ"o¿å±*SrÁ¿é8÷(JL¿êjÏÃ2€l¿êw({Y\AGNFSRQ?ïÝNÙyP?qMyᒉ‰?jæcu¿û{?n£dü'÷?P›%¡K?[ÓÄ)¼o8?ïÆKZÇL?†O^AfÃ'?jÃ
z±Ú?'T¸q{æ?o"ª	‹gz?q‡Sà¥?ìš8.-?¨téÍ=Õ?±ó1DÙia?¢HÇì~ž
?¢x‰ò3r?š"@Éz±?ïü´sºŒÙ?UA¯eœ[¨>ñdÍE1n?&'"r¶?9F "e?U;ó&ÏáÎ?ïå1ð4}X?n5ÎK°‹+?bšH™}?h×Mìwã?Pg›êÝÔ?X&Xã}´¨?ïès¾,Å?pýÄ´?U2iôI?V¶_}2ž?ZQ:,9+?i	tÌDa?í9#ë+³?¥(æ¸?°Q8({Ï?¢Ó։íˆ?˜~ZG j?'j©©ø…?ïÿ¬¶+ö~?¥æîc¸¥>Ú'u\LÏ>ûO&ׄ!˜?ûéëo??¤PòAGN3FGL J1229.8-5305@rºm ‹]@#H>¿ÙI]À:;zç&ë&À;Žã©8?°V)bßO@5Ãm}†é@,àŸ©¿èohÚ£¾Ð¿ècVX.ª¿ÑÙ9x'ÙË¿à`Á`¥AGNbcu?ïó…ÊɁ-?VÞ°HãkÆ?&xc¦uh?!°»-8 ¿?V2[cÕDÇ?UÅbË&Y†?îÁªÄ±—µ?£¹rfŸ¨D?{82Ðҋ?"¬Fʈ²"? 'l­,'h?¢ýtö§0?îƒs–¿cr?˜¼è'Œ?"x¦µâ?uðÇXÞ?¢ªÁ+¦Cn?•ÈœuóË_?ï<ˆòWv?Œ•­\â1£?O€¶Ë̊Ú?SÁ36oE?›i1
Ó²?Œ§)ª<?ïü>øÁÐÎ?9ô'¹t…?'§¯*"Ê?l'r¥¨3?7~N,òö?7V[gíí‰?ï¡à!Ø?ä=ó#ÐI?b®8?h?[±צÛ?ƒyçX‰?‹Ñ<£=j?ïq™TAj?ƒ©|Qfz_?u'íŽ!?i2ºË&X?ˆÐÉ&g,f?¢^ëB
Á?ïÌeêüžÞ?e¨êk­q?Jú'—)?AÇ,¹çy?vmźº€?cäUµ€3AGN3FGL J1230.3+2519@mF`¢G@U;{ îÙÀ9PY´§<À;Ÿ"ËÜâÅ?é¬^U©]e@:ä1Bm8@âàK¯¬¿Ðad¸«'¿å9ýgIeO¿ã߃ÍnL¿æ-b†Ì§AGNbll?ïúø¾˜?J8]ýüŽ?3Ù%¸åƒÂ?9'W¤ô[j?;ýãs
9'?ET[};?îf9`°*?¶4h±R?ƒ° ^7Jq?ŒI¬?¤°faIKA?µÛþqt1a?îǫ̂¼Í?'¨«bøPg?ˆJ¦¶Esh?;tÝ	?•A(±}z¥? &lúté?%6¾? ø…}Ñé¢?ž'˜QC_=?€
5Ût©?ŸÃÔ
…e	?œ3¨OÊ*¢?ïýR*í?+Ì÷*Ó?%ëZ[µH? 0'Ë*4?!?€˜Óh(?"óGó;"L?ïy¯¶R?^Ò&sÎ?r–~/#Â?Ë˜ë¤ù?ˆHÜì^ä?›¤r•½¥?ïló£È?‡/$ÅW³?€`å€€?{÷
¼³+f?"ôbzäñ³?'Ú¯:J?ï}ªý¼{=?ŽSeèÈ?…äځ׋?q­lï!?ubwiOA?y½DHÎ2ÐAGN3FGL J1230.9+1224@q½lºËC@R ÂÀ®À8ô>A"/À;c‰ì}l<?½óg¥<@ôÖÂ@R`0lY¿Òð‰«öú"¿á/¬i0Š¿ßÝí3¨,¿éÅN>b¢AGNrdg?ïG)IFè>?•]Ÿà‰ë?"À/Ù­?"ÕMyÛc>?jÕ8¬Y?fì'¡Üu?ígɝ!?¶éÌE•ã?§®=ŸÛ˜'?¯VÿéuH-?¡àµÏ®_?¨O‹ån2?ëÀ<¦×ù.?¬'µ[é?¸OJ¼4ûÀ?¨ŸLj;?£] :Žœ?"+¯]¥È?éÿΫ/[?°á;ë¼Ç´?µP¡Ï"['?§Þfí¾Â›?º°èÖÏ*?©¸SF?ïÌ=úÖÃ?xh|f¾ ?t֊L÷r?uÈRï°	o?T*¶×~ìÄ?Sa¥Dô)÷?ïH;´rI/?—ó‡W¿Ýæ?‰"ÌÏRÃY?'Oƨ·	?"\F!)tÞ?ŒN¡ÆTË?î-¸åº.?žÀÙýÌnå?¤oZ6|?šù ‹|¶?'j.Ùš?…bC~öNR?îT/0ˆø¦?'»Ñå«ä÷?˜&-7{?…gÒSÓ8?Sìއ¶?‹¶Š³P8¢AGN3FGL J1231.2-1411@rxž?»×²@H1ÀY!À6ÿcëaãJÀ:á\·ûe@	dŠ÷t@DETH?ûšÞ˜–?¯ñO8!"Š¿Ù|µ^C¿ãV^´ó¿í«Kô±S†PSRPSR?`*[)´	?_ʊh©U²?ïêÀáî-?cc3&V)¥?F珯C ?F$èÑ®Uþ?'©	R©æ?«RUꛩ?îƒyââ°?¸.
šÜ¼c?£,Pjüx?³U¶"­úØ?³
Ì$Ùü?¤w®Ij\^?ìü7.ы?¦Rʯ–‰?©"¤y\èW?"~£9¤"'?DÝ4gA?D'%	?ï²±'?1ŠV"¨ú?'0ꌅôÉ?~)ã%ñ*¡?P0µ
«ƒ?QãIËVÿ6?ïòžæ_šð?Y{ñQOu?E"ýF~ˆ?H㙊\?…ŽuÒ~¸N?¥4I/_CP?î!JŠè¦È?¹;×Ò¥A?¨‡¹àEh?µ™¹@|<ª?´ÐÖþœ+.?£²V^¢?ëڃޏv?¦ì¾l'˜?¨¶!ÁoP?˜SDˆ‹£?T?[‹õ?G¬Ã7-ÿ?ï¿ê抰j?r£$çâ?{|ëSñ¨?q$$žž¯PSR3FGL J1231.5+6414@_ qÁ
{ê@J`»oÀ: 'oÿl\À<PœÐ…¿?×Ì°áù@2ugMA?ÿwß	»@¿¥' x'Û¿×PÈfØôp¿ç;Cɔš=?Æ4U-j,«AGNbll?ï¤E©¤Ëô?«ý·ö,ë¼?"2'ȃ€j?¬5zëk?Uãn'Ê4>?RT碋ç?絛¨=?"s6Zé[?sƒð¸(î¾?w	½~YR?w$;:=?}#íqeN‹?îÏDÔÎ×?œÆ-RFêb?¢c[óZ{?™Ò'F‰³:?š_wÑ÷?†Æ!7S0?ï;—+ô?—[n΅WÅ?€•~š£N‹?'ŒÿÛ¬‰?B[Uwfû?þCô=Øg?ïœÂ±U?¹Ñ¼ö•óó?‡|ƒél[?¹ÕȼûQ"?E,ü¤_'#?Aûòkþ?ïâ,XV5õ?jª·CŽ£?]T+,Qã:?`'y6ãš?^S#³ÏR÷?_O¤‡!/š?ï
è·Ñ?Œ@¿&µ»'?'UœäÐð?‰¼³PÚ 
?ˆ"°Éùî?t1Â¥Ã|Ï?ïà…ÔôA9?r݉p1?Yš|ÓC>-?bóXØ)fr?b¬ì ½P^?ki"1›ìûAGN3FGL J1231.7+2847@gÙü?O@UV™¦5À82~5ÅÀ;
3Ï:eW?ã쏪yÞ
@C¨×¥ý?ÿ-À"!¿ÞÁ¼š½ ¿àÞúvÔ¿Ý7ÁÉu¿ßÃt|9óAGNbll?ïû֚Mk?=›'V¥Y‰? Íö預"?pO§"ÐM?8ä1A¬?9.ü>a?ï;t—£í?¬O-&ä!P?l(#à,ð?oåÈÉ>l1?™kO,¯?¬ÃÿÂÅ?ïudAaä?®råÅ?wò_o2²?o"ÕBè¶ü?†ÄÛ39_¿?}wKr?ï#Ô¢üf:?¬œ/êâ?h쩽ª¤?eM00³Ö?˜gÖ}ûƒo?)‰_fw?ïþ%›6ˆ?%¿!| ?̎H£{C?ŸZ@?#@'÷»?"ź&ÍÓ?ï͇®pÒa?†2›«.?Y?ÓK_X?\q¾±É?rì3Ùò^?…øWÞñå?ï¨,Á¡lï?sõPÌ!´?ql¢§¬?eóQ4¿¿?z|ükP$?n-rœÝ`?ïÅgX(àõ?kÎf a?YL1ŝ?I¡UÄJm?vùGr»úd?iñ`AÁãAGN3FGL J1231.8+1421@q¤˜ˆv\@St÷íÀ:,÷öFBÚÀ;¼ùS="¶ÀŽ_¡¦-|@4Ö8±Li@…=ÀªÕ¿âqõ!¿ä+t¡´è¿ÜŒBX•¿äҏ™AGNbll?ïάtMë×?xı"áÒ$?:À³wº¡,?5eR[Á×?výº¼$â?wè;Êé?ïvB´Qù?®L汧Û?mW»Ã-i?nºjÖ×Íe?‹cÿ-ó?®H«šù?îäÙ?ï%µ?ŽlV¼æð?"¹"C›¥?u±Z?™\Þ) ?‰Æ¼]+
Ò?ï·b	ŠmW?|Ò¸îñM?$Û|ZÂ-*?/ÊÔ3^èÜ?Ô§¶êm?|¬Ö|û£?ïôSÆÈô?W5•wU?(nRŸïäƒ?"y+mIã?TJ§ÐµUà?U·Î8¶ÃŠ?ïÝlÎúo?~ ½ªcù÷?VÀDùQ	?W_7§BðÝ?g3#º5˜®?{ƒØåþWÏ?ïŠõJ€'ô?x‰8XÐz?tpû¦æ‹?[‰ß–Ä?ƒ
/|Bi?v
"¦Ç¢:?ïó6Œ•5m?R»àWvë>õšÝ4[ËD?S5qž‰?Y<{º½?R£IÃÝØÀAGN3FGL J1233.7-0145@r]cÿï9@Nf­ _À9úö«ÃhÀ;{µò•´?ÙÝW^‹§@üsƒôl@ÅhpM›¿åÚ¯/û<Ä¿ã<A"<ɿ㖭gÆ|•¿ÒÏç&×AGNbll?în)Áov…?§dÂ)L?…gí±1:?‡kÐíõ?£Ãh|ċ[?¥.–‰wk$?ï*îk??¢(Wý‹ê+?"Û]oƒ?˜KŽÌ€?ˆ{ᑙ´¶?'‡¡/Ì1®?ëó[S°"¿?¦¦]#Š?¥Ù¬âHJ?" §{•³Â?µx˜
Ãëa?¡[õŸ(û?ê»Zð¢¦?²gZ @?©ÚÔªð6½?§­!'  ß?½7¾%r³Ú?¬…¥qÄ1€?ï—Hšè=?ºLF1?p}	é×UW?s.F-©²?ïTJ%Ü<?‹üxç}£?ï½»Èv.Ž?‰*¼x3ô?r+mFÏÓ?'`CgØß.?mí]bEX?uÛÓe~È?î‰7¿W?",2PÎ?"»E&æ?"ào®óú·?›Ð½È".?Š'²d…?î4Ø
(ß?'‡ÿÞà>?'¡3î|Ç? 7Vz(o?š¸UŤý_?‹IC)›:÷AGN3FGL J1233.9-5736@rÉf?šIÃ@½ËCòžÀ8ÊÅ­ÚÜÀ; Îô©‹¿ðØOÒ¦*¢@Aˆ£¨U@Pèß|ý­¿æ¢.§n¡¿ÞèžÞä
¿âÿÉjä¿ÝE?IR@AGNbcu?îc¶Þtm?©"ê5îmi?wcKNÌY?q¬r8P"J?¦Ø ¬ç(?¨x_Îväò?ëã(Gó?ÅcÍ"Òä?'O[Öí?™,ÅuhØ?¼O¿ÆTÈ?Ã/yüVŽh?ëZØ®?¦š|
Æ
D?¥júí
Á?oäà‡?¸ß±›Œñ'?¢½»³ºP?ìOÇ£›¦?§cñ;î£?k}c jg€?k!£FÌ,;?¼¥ÜT÷u?§HDGš­È?ïäßñ ?¤û—Ú_"
?n"aqd'@?p¤ÆC©Ì?˜[—3‰³?£Ñå³M ?ïë€þ(v?§-µc_¯?u}kÔpˆ?€K䶹ù?˜ƒ5%½?£¿[ˆÝvÎ?îrŽÌGR
?"w¾­™8?"tÄ1¤'?ƒ+¢SP+á?ž™±²ä&?Œè¶
´&?îäÿA¥M?‰æAX‰Ö?Gõ›v)?ApñEO}'?¡P7ÐÑ¿%?‰ÂdÅФáAGN3FGL J1236.6+3901@a&°)(@Sm~ßÙïËÀ:~1«s¶±À<
M`Ûã?Ä¡‹Sc\ú@0"[—*@ï·¿ttœ¿îFK­—A>¿È:́ʿã—e{ž¡¿Ø2Ÿ,´¯AGNbll?ïõ»FE<S?QîΘ""?@'ò!¦¢?A v°¯ž?HÕjŠÇ?J$ÏIè´¢?T‰Å?ˆ¥Ýjké?vÁäÌ%è‡?y ÞøÂu»?€/¸¯Ÿ?ƒ=5àP?îN©Ɩ?"4N]¨t?–wi'¢Â?ˆpœº?Ÿ°&"Š?)¡Qܲ?ï.3]5Ì?lK"m"?‹x˜È,aÚ?‡gcٜ¨"?ˆÿš]?ƒ_ÙzEó?ïúҖ\Å ?A,œŠ†.$?2Púóó?2j _?u?7Yýd(ú?6}-±¼.?ïÚ×zûŸ?rÏ
º?a¼ÏYê	"?e[|ºÓV?d?Yž¸L?c·ý"fâ?ïPâï?ƒ°t/ßb?"7¤y¡ø}?yäþhëB?‡Ã»½?zMðß2Î\?ïُ?šìø?gPIb'RÁ?hwªTq?Y'.ÝÛ·?\²'´\6a?_8,×$FAGN3FGL J1237.9+6258@_b^AÔ¶¦@K
q VL=À:Ƽj~ùÛÀ<+Š«ÀË¿È;Ki¤£'@% ¢!}~?ýb
Cœ¸¿ìُ&_K{¿Ù¨L·"«¿Ön°Ëu›¿ÔlZÚàaAGNbll?ïÃ@Íá°ñ?…ì!)ZO?{Âém÷?…ooS¾Ñ´?JÖ°ŽEV?P×ìjô[?ï–8_(?Ë?‹;RuõxÞ?x¸÷è5\?}gåóáwø?|ÓjXý?'£($h•m?î\/Šuþú?šnD.°ö? H3‡'E?™ýå‡Û`?"駝,Æ?H'R螧?ïxµa(íh?‡(Buӗ?moˆt?sà®Û
?ŠvæSkò?'—æKß?ïä™nóË?tWm"5ë?dŠÞŠZi?qª±a$ž?KnÊÈ7ÍQ?`TSø¦H—?ïà4ø҆˜?k-Š>•6'?]ûw1"?aú"ìEâÝ?`ÍKzå<ó?`ŸÀc€­?ïÞUzÄ?"í¾æ®jú?"ÿËCYh?"Ð…[L–?ƒÔmà˜.?l¸°TØߪ?ïæI"±Ÿ?`%"
VD)?T5VŒ~?K
ò*·*?_7¡Pá?XoŠa£J&AGN3FGL J1238.2-1958@r«f?šIÃ@EcêßÝJÉÀ9¾RsjZèÀ;´'¾ÙÅ?ÖÍ25K*@)ìþñb-@ÊÀYY¿éå-¤Òï¿á©ÉÆÍ¿Þãµ¼ºÛß¿ë¿öAGNbcu?íÂfxL?¬àõü*I?±U2kÊïÌ?¬˜Ú]ØC?cVL	
Zà?`ˆ>ÏßÖß?î1Ýñjïk?¥`ƒ:îÅ? ¾ÏRüq?šÆåW2?˜F£5KQ½?œQŽzó	y?í.S}*£? Ã³¾Eæã?©óóo]aÙ?™pk4òÊ?£&ÔÁh¶?=ѽd‰s?슰êæ_½?¤L\å^>$?ªÑ¢•-ޑ?šۓ´ß8?¬ƒN»>›?™ìßÖd²?ï{CƒÉ‰Ý?'«YñŸ%[?'/ÖÁÜ?'4´:û@¸?JÎô&…?G5Èü$‹?ï†X9'?"zšÁ
b?c³¸çƒ+?yđ¦f?z{ñ¸sŠ?zŸñ†šUX?îÈb1"?"xòRÜ?˜•Ä¾Y™.?Ž–gc{g?ŒÍýãbi?€ZWíÂ?îÿß{G–d?'ñg®ád"?"kÎQ©O?xôõÎ4i1?‰0"‡W°h?vÅzô?
üAGN3FGL J1238.3-4543@rÈÇ`|Aš@1cÀ™¸£À9Îä¦f&À;©:}ªP¿ï™£ÒO)@|b¤dùª@9Ê?©¹!¿í¿:ÓI?¢‹ºÖ!¬š¿à'n¦`ý¿åÔórFfAGNbcu?ï÷Â2%R[?Eó™ñ@Øz?>‡'X¥G?4àײì÷ ?A¯sÝ£N?=U Wc=6?ïE¡ä…•?
ƒdï…ï?rEÞ>`Ï(?oIú³Ü"/?ƒ¨a~ç9?ˆð'ŠíÀt?ï=êiÉOó?‡íõÜþ'®?‡?ô¾¦?­å·òx˜?‰~%¦«ñx?y'öKlä?ï‰áéXc?'?gÄÁWÒ?`Mÿ8K?`µÖNe
?‰¨d)ùE? +ý0Ž?ïý	Neò?*Mq0u½?%kÁZ"Žè?ó´=d?(ã«äL'?!ˆ§fô?ïÓÓ'ê±?v
%2íz±?\ã}kÐ-‹?TT¯,?mº~ݨט?s™:!"¢ ?ï¡7#Çt7?{Z´÷®û¾?wÃ!š‡êÀ?u‡Üy†]a?w¡L‡íE¥?p _̼WD?ïåÂíÙjs?`ë#ö@?4ÃßÞöú;?2Û»î÷pè?g¤–M5õ$?_xN¨ª¿AGN3FGL J1239.4+0727@rc}sÉ@QˆfxÀ9½â¯ åÀ;§†_*2¿ñŽÑú‰ @j«Yàq@.Bß·7¿éÓì$<0™¿á@­åßuú¿åì''GK¿ã¤	"AGNbcu?ïÐ`ىŸ?rcôŸËé?iÐ3%¦ ?j"ƒ¾éšÆ?fk÷9ÒÉ?cÐ~§_´?ïœhmŸB?Œ€Ý=»Õâ?w,/Ø}?…U‹îM`?zŸš(yŠŸ?~ä{çI`?î@u7Ü݈?–iÆ07m?–ŠpµÕÀ?‡£H…Zz? ³t{Æؔ?ŒÌN˜V‡þ?ïÅBóMH?Œ.ÉdB?pJ«.ç?n§Ç;‰µ?š!"ñ'0W?ŠÚ£‹F*î?ïò'1È$?WÊt)0ô"?J.9´¹©?K'öxíÑ?M4ÿ:§KÏ?L'XböÀc?ïá*¬à&?j+Oÿr?]0"ï}1?_ÆÂ#Û?`=Jˆ"¹?]âg¶l?ïbäð@U—?xUTi½tœ?'Ÿ&Zt?oÎ.Åd÷o?…3$^rëÊ?j¨¢™{É?ïÓô¤µµ?g×´*>?õ?BUy¬$?8Z§|?sºþTjv¨?fÿ»käE3AGN3FGL J1239.5+0443@rs‰ :2+@PÚqÿ÷œ"À7'Œö(/À;¢!'—ô?ûuëæmˆ@ŒIõl~.@í*#•‹¿ágï¨nô¿å¥9¤¿æfâN3Œ¿êîÀmvƒžAGNfsrq?ï òb~?ˆÊC(ËZš?ƒÍvý¢¬?"ÝÌÝ{x?_¯Eå&߸?|
ÑĞ#?ïÂVÛȬñ?‡);ÚîðÛ?m\ÃàuP?ƒËÈp¿¬?p&0Á•N?rÇé!7ü?ìá°m+ãš?¥ݨ´Œ?±Ãâšà×?¢2²ê)}H?œºgú£]?"Á
̨Vú?ïã§,)S¶?sÆà²Yob?C+o9™Dj?Wg)1¸?g÷í¿c?r–U(eÏ?ï̼D¥‡ ?t/œ®¬>?u
{6]±J?rlÀœŒ˜ø?R]‰ñw{^?T°¥Ð
Ñ4?ïäˬ;\Í?j
9"(c?X_= Ê¿?W¯›.´9S?^	i³[(?bÙ·I{.?íåÜ?Eï? ÉÌþUC?©lAÕ_?¡–"á·?'¥wÜ  ?Œ´{n̗?ïú) À?ROãGVŽ?0'7i¼ü?6^—ŸR ?>ž«!D?P¡gJêBAGN3FGL J1241.6-1456@r¶a_Ìr@Gíù?ò^WÀ:C5'Ì÷À;Ækš'Í¥?â'AêÂ<a@º¿-§Ù?ÿYÊÿ˜&'¿îhŽa'&?žGь
v¿Ôyµ€¸Í¿ãé<¾5AGNbll?ï÷×<+C?Fò«:àÉ?@çƀ1¡?:8â-­«?BÈÛûÌJË?<E]-¤4¸?î-vJµ?ª3|BìoÈ?¢7€íÆ?¤:1rFw?–Ç°+É?•Èío‡?ï""B€"K?Õu&ðr?ƒU€ÔŽõ?n»Çv?'·Iؼ?yfý²Â8?ëþ–qØÅ?ª/ýr×Äë?³z˜#W0?§0w"*xx?©!hšô­?™Øð[B'	?ïûRhŒ?5a…¹tZ?.ÿ'0Ö?%ÎÓÉÞ;*?6f@®}'?,¨nG"®?ï‹$¤'´X?ˆt±oß?€áà¬ý?€ëRߔ?x«€"…¹?zÉßàåXk?ï‰1¤_<É?n [0ҁª?w¬ªB1F€?^v‰ØßR?ÝAÍGv'?e¸à¹@6}?îb˜%¼q?j$±Ç*$?£¬htкØ?ˆÌ5qR²è?ˆ¨Tö¼_?w"Þ§?ÊpAGN3FGL J1241.9+0639@r'øÿûÎB@QZýç!À:{õ[aO¦À;ÈÎX%[?áTr^÷Å@^wڂ?üÄþÍ%?Ìqƒ£Á™F¿ê'äjÎ*?¬`Ÿ…ŸoO¿×åï!z=AGNbll?ïñ5š@³y?ZE.ÇÛ§?#G¦7#f?"{'°ÑM?[+ÖÓwë?Y[VŸ÷"?ï®
ZFó?‰8ÑFâî?rj/nj|Á?'"Y|[ºÎ?v#Eí±‡?{?±—¤cX?ïÀ¼•"?‡ãv·‹U?"ðîµÂԂ?v)±mÏÕ?•‡p'³M)?4õ?.¬w?ïPŒ×·?–ce[ø™ò?fb=g_¤Ç?u5«!5ü?š¡ÎH,Qˆ?•?ðæ•v?ïùÍ&õôJ?Eqìå'×Ü?ÝØÅäñ?eŽ<îÊ?E¨FUQ?C–¾ˆL?ïäžM'?e¤æƟin?YA5¡ì°?WÄmýqZ?]'/['‡?\$çs—?ï'坭g?s%¸mdg?wd]¥µI?aI~G²\æ?ƒ"iä24ª?nºFÛ¯/W?ïÈÙï[SI?t&)Á¹®?f…Õ‡H?a5}sée?pPAQ%+ô?nðµ®Nç­AGN3FGL J1243.1+3627@`¡aՈ]@T Æà#Á¦À8i§e47?À:ùP°ò{³?ËQcøšÓ@@쉫æ?üM$þçüÿ¿Ý£!%G?ã¿×¹O»¿ØZé[!ܿӕ¾ùiRAGNbll?ïáE"Ð?d}ëº
à?OT'žV(ö?I5i= Ú?f©°Äµ'?aɲԼ¤ó?îÿr­á>
?«ÆÙùÉ·?yùpoƒ?…¥$)d"7?™ÍF"…?«–
eV?îSz¸¥Dë?œyÆ21Ÿ?ŽÌu2©m?"ðº&]á?£Lšò»ó?—¬<rm‰?ì¡fLe3`?¤˜Ç¤©I
?ƒYˆͨ? ž'=F¶?¸‰ª­ùE?¤/ÄO¤?ïòœð?R°†Ù˜?@(k}9ì?8[Ý¡èº?S½i@'É?N†Ô5T?ï«0ÜÛ|'?"OŽ–¹É?i'5cB|H?yn¢ "?}žvÁ#?'å$ýþW?ï6£Ì^¤?‰¥fɑ»?'
è²J±O?v@J7!¥z?& YŠâ?ƒ£¦?È_?îæUrßVÎ?‡±Ž'×|­?v.
+á[?cŽùýç\Õ?´ÆÖðè?‡"j;œ´AGN3FGL J1243.9-0217@r±µß덂@NDÿ΁ÙÀ:L}qDçÀ;Ð:FLëk¿Ç­Í‹Â&@t¿CLZ÷@|Ñ`…Pâ¿çùÄ­ù¿ÞÝD3[¿Ó½°"퐿ê"ìiSAGNbcu?ï´ßq??ŽRµHeŽ?€™r›Àº?‹LaY@¡?S«¾¡D@?a ʎ=X?ïmÀ»;3?‹¬:­'Md?‰¯ô~\q?z€lÛ£9ã?ƒJZàë?…Ã.[‹?í÷‹ùc•?ž(bWŠ–Ì?¤Iü7ڞ?˜× XÓ+?˜|lF¬
*?‡ØÇ_ƒ%í?îùì?É?Ñk•m?€†ˆ4"?zK†/<U1?˜p±?"ï?‰Ò+×*f	?îÿ&2¼X?Âk(·^?˜áþ&$ñ–?½€wãÖ"?|äî£Ý¿?¯m=Å-R;?ïӑN¾ÌP?lÀ;ÀZ®Ž?f1!@- Ú?_t.J ?f=Þ©öã?d	P:DêT?îðG™OO|?"š`•¡Oa?—Ìö'µ?'ÁÓSâpÇ?"ÒÆ+…?{^½ýˆuÀ?ï¿b: §?j1à¼h?jbëâÆ?X9žçt3}?s×·¥ˆç?dšÃ@zÃAGN3FGL J1244.1+1615@r\:¿¹¾Ó@SÀW_ÍÅñÀ:6—ºœH¡À;Úe€…¿þ˜óï{xq@fÚ`´Ø@i1€«Œ
¿å±‹I¹vH¿äú–wâJõ¿ã*0¯dÿ¿ïÿÔ¸àÕAGNbll?ïÂKÁ
j»? mP¸Å§ì?X¡¯aG?z÷0_ƒ(?xÒ÷¦'ì?~Høo?ïnç!óÖã?—ýXîŸ(¦?rª1RA›?tDÇ˪9¯?ŠñèW՚?—ʝ&ÿº?íք†Œ÷?¦¶;ñà¼ö?¡ð
	$'?ò?֍H†?®­ý¨?¤"Q§?ï§ãÈ")\?'HSø?YÆØ6Ð[)?e·"e`z?'Î2â-Aº?€±ö>Z?ï‰GhŽ"²?¸p¦OBZ?b%÷»Ùφ?"ë@¢©Úý?‰$§á"G½?µ)\$+?ïÒé¶+dw?€TN¼(Í?[6…÷õö4?\ÒÓåVn¿?o{ Fö£?}ÔÉ˂Î?îm˜h…ê)?šՐ(?–ú×>n9?‡®û_ð*?œDø+¶œ?–'Ó=7?ïñ±AŶó?]…fѯ+o?‹*¡"¡ü?-²ÍÈB˜/?Z¤Ê«cK?]߬AÆAGN3FGL J1244.3-4955@rÜ7À*ýÛ@)ÛҁA³ÿÀ:vãŒ+óÀ;ŠW™¿Ã?†Š•'@o"9櫛@{ÿªÅ'¿ê¥¸·Ó&¿¿æ[±9'ó¿àÃùòþB¿ÞIî±##AGNbcu?ïí^X·'?^™#ê£Fö?5g!áí`?2þ¡9"fˆ?_é‹7î¼0?\£"<¶_?îæ{`Àh?¦;sá#F?}Š'/äêf?zýDBˆéY?›Íúà‹y?¤aã2µvÿ?î"ow\-?"Võ$ò¸ ?Œ&ï	;?zÜ>ø=ßÏ?Ÿˆú'¶^<?Žrÿ•»­Z?î˜Âó@e1?'YUˆ|ú?b¼žž=?`ê%7ø›?¥Iÿÿ?—xƒÔžC?ïÎ¥l¢/?®RU}ä?T=­û9¿?†§V˲©2?sžxNb:?¨üºŽýK?﹇¿Á:a?"4—ç?c)¼+?bËUå:?y§W¡f	?€PÈ' $È?ïw\H]ðT?x	<÷ý‡?zýÌ{Çã?l`ÐyN{[?"ªiuy/?p[#ž2%?瘟,õ¬j?pZ#ös÷?VE}€ŽÒ?Dgm–õñÚ?'Ž^"•?on-¿ß´AGN3FGL J1244.8+5707@_. {5+@Mýþ +ïrÀ:PÃë|»=À<¸e6»~¿ØšËOkšz@(=}¥@½?fj¿å£éqè¿ß öÍ0 ¿è½)¼<ë¿¡X\|F'AGNbll?ïá\ X¿N?gCü;Ît?VŠP0?WKÇȎÌ"?ccšcØêU?aÄéx±ò?¢;o?Ž]csÇìÌ?vÿ˜òï½
?'—Սm¼?z2•÷Ìv?i?ºx1û?î‡hdBtÅ?'J˜Ÿ5Ê?'ñ½5ï¿Û?'™AÚà?!6Cyu?ˆ—T—rR!?ïY†¹ÃÍ?ŽZ ç?	˜?n&xÈ
Tb?rõ@Ï¥Þ?'
Y§—à?Œã²z7¿å?ïõ[Žh…r?R³gr>Y­?;˜TXW!?@Ò©¬Ý
õ?My˜)WF?K1MF§Hð?ïäs;>£?mìeÕ+ü?[‹~i¢|?d@c¤ín.?\7›žë¶Ç?]#÷µê?ïN"{u?};Å.šž?ƒ";ØZ‹ó?rò(§ð´?ˆË¥w¡¶Ä?sI«œÜ?ïëE$f*›?_ÃØVs?@uŒk€#?<IŒë-a?`xH«ˆa?\"lєþ™AGN3FGL J1246.7-2547@rÙÈ¿Â"O@BˆÄ`Á
À6þBÍ*1À:Ï;+O9#?ûpF™ @"±M?@ŒL/Ùa†¿ànK¾´9¿ä"ö•Ú-š¿å˜©PŠ Ç¿é+=}[lÛAGNfsrq?ïÚOßK?mõ>±ó?cÒx ¤F?fCÝÊ%ö…?b8ñžøX?bgÔ,îò¦?ï½ÃÒÓ!%?}÷L~èü?lª¡á"Þ?líÕèH¹
?rÈńðœ`?uÕÞÅ?í"ÿ>¹ú?¥
vÎÙæh?©AÒeñ?ŸDψú÷?œì[Oµ^—?–ŠA£=¦7?ï¾eÁ>¾?…]À†Š¡™?LžK ˜"?e§ÝŽ—Ü ?}`Ћõt?"oŠD¦O?ïâ²d§Ü?j*-–ŠGL?a†•Ñçê?c•"i?XÁqa…˜¾?\¯~Nä»h?ïâ"!æZ?iøbuæ?ZùÔpóÆ«?Vefúqˆ÷?`aäؒ—?c$öÙ·~?îP¤KÝq?›œ³²ý÷E? ò€e–è?–P¤! Ñ?"{§è¨%?"P0Ú4?ïò?AMA?d/œà&ïú?9šøäÚå&?8¨ö7æ†?U¾ßܙ}?c–¿_QûEAGN3FGL J1247.0+4421@_fwž™@R0Ÿíp±À:šF…öN¦À<^â
¦²?í¯2½T@7—›è~@wå¿·æa¿æ9Öi>ï¿ë¨6ýHs?»(8¥°K¿Ó7âÿÐAAGNbll?ïö®Þ'àM?Tu‡S4r0?5jˆq©!F?75Q·?JBBZé·?R+ö*­?ï¼9:Íö?Ygžv'{?m^©ÍÔÅ?q7ÔiŽò?s4
¬›"í?v›m i±è?îÉ!"_Ë?"«F´'6?Œõœ:7þ,?…g0í†÷C?˜aW†?÷/ !`1?ïÅ'6¥®{?"2‰á>?V GY˜5?pá"n·a¹?wÄRôÿNà?€ž°±'¶?ïûv ñ&É?@6ƒ=mcþ?*hקíªs?*Þ謀?7Œ~{(?8#,ö¶¢"?ïç¤;wê?eš$©	©?Vá.ï"Å;?VaVàvÉ?Z÷ˆ–˶³?\*€v?ïGÿòؾâ?šÔºÔh'?€ë²¦'ô·?…A#ˆ¾?P¬Ü:«?‰
s÷lµ??ïñ±âKö4?c‹ü-#®?QßnÌÑ©O?^¹WS2?Ey˜ÁjÈ?Nö°í!AGN3FGL J1248.0+5130@_Ž`€sX@PgGÿÞrÀ:"HÊt,ùÀ<­»§¿êç
`™P|@ç	ç5@N¸@xÁ¿ëiĦ¿Ò|ҒÎ=)¿â&|§­¿ç©	¦ƒAGNbll?ïô¨ï€‰†?[ݖ*?Q]ùANÙ?YݑÄϯ?5@Ÿzœ?-1ÛzË׉?ï£Îñì?Š·³ÑwX?tdRøcì?'êÇ´q¼?z
ņ¢?}	LÄÒ?ï"ˆÕjïÒ?‡…¬Pdù?Œ<†šÖ‰?¥8¬—i¾?‹!±,g¤ð?xnvì͟?ﲉ³%9~?xóâ@?d'êo"÷??`'€uM5?|§1-Yµj?ugsDÛÓ+?ïüí?DIÂ?0eôÅÝR?.ƒ`æP¸?+•²ËÕ¡±?"¨ªÅ0§¨?ƒj•˜?ïâcù_ãü?füà±C?ZT·ÐZø?VÞÐş ?`qªð·–7?`.ÂP?o,ø?tÓçjȱ?zû˜ôÏg?p«¬=û?y#{žF¨Œ?h¼ÔWÐ5?ïó·	
'1?SÙiDêy1?:C9 WÎ?2#Ë-ÕçN?RëՄ?R7ZÁmAGN3FGL J1248.2+5820@^îÊâ°@McC hÀ´À7Òæ±z`ïÀ:ÿÕHœQ?â"èç#~ú@µO{é/"?ÿ(«Àb±%¿Ü1\~†Ý¿ßԒ;ßÝ©¿Ý…9ÿïÓ§¿Ü½œóì zAGNbll?ïê0#£?ej¹åÇù?I£!Z¡b?F&Óê
z?_ZÙÇß?bÔsnfì?ï
D=¶]¹?£ˆ[Zy@?±c¿áåŠ?›ñ+Ç?Œ)Ŏž?"Û¹%…]"?íÉíVD? í´O²­­?•t"Tõˀ?Žó¥W&¨A?¨³ÆûÙS?›óÈ-8™æ?èI©Â0½?´ò»r'&ð?¬%=,Ts?¤6håÐ1?ÈyŠbôl?²ÿ¼#·^3?ïõN¡"Ïä?WÓë÷;?:Ðiž`ÑÏ?EÌ#hŠÝ$?M]Fª'«Ž?M±¦Á´ø ?ï˜Îçás?"(°´y€?|w¢Þšµ8?Œ7¬kb·v?w!HA…W?¥ƒåýq?î9'v.t?œˆó!¿%?"NÜñ'ð¨?žð7ä\†?¢¿€"'#a?—	ÇÅub?í6Í~ùZI?šÄŸ°º\?™'ÞÄ,P?ƒp]ÿó<d?¯ÊžtD?—"b»–WAGN3FGL J1249.7+3705@_6ÆÞvB|@Týß=À9³ªŠ'¥aÀ;m¤K¤CA?ñ-
¦®*@—üï)n?úx@HŸ¿ïÿÒ~p&?ïÿ#Ý"¿Çzß¿Û­KÄ	ëÍAGNbll?禮â÷þÌ?†}¼GM]?|sìGž?~P|¶´-?p1Œ~Kßû?v8Ãî:[u?í¡Ò?¼%M‰.g?šãëªæü?¬}坣ö\?¨|R-kÀe?·tÝa?l?ì
ÇLŸ?¬¨®-}¥?ªM$E
Ÿa?œ
X[|L?²lı?¦i³ÒÕÔ?ë¬^#»ŠÊ?³)`Ǻ?»L6`‹?±¢LUúû?Cb@?œN0¨?ïÈâd/Œ?€¡õ…–?rO<«
©?tYö>ÖÂ~?b#þ¸.g?qj";º…?ï.Õ7vÜ"?¥ßƒw&? y­£	X?Œš;øK"5?'•?"k?¤¯cJ÷!?î6:='[?Ÿ Hi¹»?žÃpîÚ³?"+¨Â"Þò? ì:§ í?–âBuˆ|Ã?íâ±f¦
'?Ÿ'þӃjñ?­ö8Óq†Ê?­+ß¼E?~õ†žÕ?yù ¤ý†AAGN3FGL J1250.5+0217@ræÀ]RÁ@PJ¹ßõž}À::¬¤8À;²I|JÔ:¿¿$b#ÐXŒ@Nò^@Ÿž¿ô!P¿äF+"Eӿ祐¾¤¿ÞmŸÌtÉg¿Û#Þb\§²AGNbll?ïÚ;¦°j?t**½m/@?C´O±ê=?C¦b×^d=?p|X2
?rà<6®:*?ï«A¨¨'?ˆ »?êMR?sÿ€¬ã?ƒM§l"ÒQ?v`­Äž~?x옵'?î§÷Ë~4?'ŸFŒd°?Œ
ù¶ÃS°?}©×±*¥ˆ?œû‰­ü·?Š-¸ùDö?ïá³cÅ!?Ž
kK¥c?nhGº•?l3_uRßÃ?›ȐÊ_'?Œ"=/ï˜?ï÷éx šw?L)mcΟ²?)؅¦É
õ?&©§Ú¼ÃŠ?Iãý†šXê?IÑ¢6±?ïâFcM?k?™Þ?["¼°ÿv?^.Ù¢jC?`+žYëÛe?b§ú•eó?ï…@´P)8?r	qOñØg?xŠ÷ÞÔý?`Aõ}ûðZ?'®
{´óe?i¸÷¦?ïÐ"ÿMAk?fÃʳU¢?WÑí"^Äv?FŸ\Ê×ó?qúݚ-s?d©yU=^"AGN3FGL J1251.0-0203@r뿀ß×@NhP`j£ãÀ9Ûs"u"*À;²7_ÞO?ÛdÚ¨¶ @&°™_^@ùf!È?í£Îxoê¿è±úŽ|¿æÆ÷ ¶¿æ¿Ê+€ÚAGNbcu?ïû¢° ?9BL3géý?0ÐS	ƒš?.*'0í%?2-2H`ê?2‹V=øú?ÛUë^?ƒÅ¯½–{?x¤…R·?"‹á0Å7?~
EV'?'rÍ&·Ã\?îÝXY͵?''9¦uè=?‹¬@~ƒ?€f¡-?–†½…\ ?WÅ1úƒQ?î)°Ÿçß? C†~¿
³?‹ý²Ùí­Ô?'¿OÙ­–? 
ø>ª/ ?²ÆÇn!?ïþdLí?&ÇÃö©Ýç?!uPêÝÏ?¾¥ 'h6?+ÃûÆ?9Ȥ^×&?ïÜÎb¬¦?l?Ëy;j?]ððâ"~?XèB!¢7?d9$õ'ìÄ?eÅYàIíç?ïhAjn?ƒÇ´um3m?€Zâç¥Çù?vtE)ύ?…"ÛµA«?€Žÿ\Ka?ﴕIŽûl?zÓGÿ⽔?nf*r—' ?]8Rì[êT?v'Fy?xxÄhÎkKAGN3FGL J1251.3+1041@rî-?ž{@RcÒtwÀ:ä9ÐÜ&À;ÃSP	,Ï?ѧâõ$§!@ÿ™©ß¸@'‡?Ïε¿êiMk¿çõ'C‰¿×.FíØ¿¿áX•:íÅHAGNbll?ïþÑUE?Ö}²&"?tü4*ö?ދСüö?$˜ÝVd?õ¹½»y?ﶠ)øï7?€yò
Q?o»ovûø?pÌÀÉØ?tÒ`À:–?v÷'þKË?ï[h{?'FD)r­?zh=]°ï?sÜ^6(rp?‹÷qĜa?zލ`›Œ;?ïEEçZ?ƒxçpÆ«?bۏ¾3ü?eµ¡¥À8&?‡÷×ëÎj"?€Ñ ¤ÔJñ?ïÿ(ÙVâª?Î
þ`8?ÚÝÃÚë?eﶌ÷£?©ß8¦Ö
?N¿ÊÖbÍ?ïäjZ£²?g]\¡F"D?Y³¸Ý4W?X"ÇWÉg?^3ïPÇL?]äƒJd?ï¹£&€G?oqW•B?jŸøˆ.d?dgk~?v!-úʙ?eÚ1éIî«?ïç¹#ïë­?\üÐöÕe?S¨Çö€z¼?Cbh Ê8?\äï¢÷{¡?XFKWAGN3FGL J1253.2+5300@^"®ÀrKw@P9ßõž}À8U'ÙŒÀ:Û«8þNO?ôE!óé@µ¹	÷P?ûæÁšê|‹¿Ö×,>CÔã¿Þhvšò¾¿Þ}âw­¼¿ã8á…ÁuAGNbll?ï$@íc£Ç?•Çì¿æI?"miR½†Æ?†'ò0‹¨?'A-¨ÌëÀ?2ËT2Ïd?í0¡KÐÊ?¶Î)'öl?¬Vä‹?±ˆ°Á'.? Ù"aoˆX?¥¯ÊkE4?ìã"u©Œ?ªÆɁØv"?¬9·x% c?Ÿ+Ö».?±"¡‰ýð?¢nr0kz?ám+K?¶1™>b¸È?ÇäfwêXŠ?µ[òž\eË?Ñöòná£ã?´C¼ãã¤1?ï½Ü Ÿ)H?	܄É%•?py?‹Î\?w鈍²Ð?p˜°#=ƒ®?nµYf?Np?îé4o{ìh?¥+‰H8Š?–ÞuŒa1? Ö‰å̗?‰±'2|‡™?:§é
ž?îc"ÙÁe?œx—rKB?šz¤N
?'Ÿxùå/?™Œ¢K€N?'õÒ?æì©G?¨èÕÅXŠ?Ä¢/?¥wK/,ð?À4™´vó?¡ϱŸ
AGN3FGL J1253.7+0327@sп "`@P•€	¥›À9o™YعjÀ;^}Vlô¿ñdt
Ãâî@–«†ñÌ?ýwý%	O¿ÐV>Zø¿ß-‡Ç#¿ã,tè$Ë¿Àº½mU»@AGNbll?ï÷Š-ڞ?HYòÚés3?8²Œ)*bà?48bNT"ù?E0'<oÇ?BX…®r•Q?ïÆ\Ìn›?{ÿQ`›"g?gµÕËâ3Â?k%ë¤aÊO?pö®óÊôÐ?t	_l"›?ï(†6)L?‰B¬8\ܳ?‰"3ËM_ž?€ÌJ"C‹'?ŒÜê±w!n?€ÇIH?3g¥E?'õmˆÏ0ý?,9-Ó<¥B?1Nšç²!?Ž"€ríc?'Ø ÖúÏ?ïü(cª'?1äôé_‡è?+,òk«ä‡?$wGõ=à7?1)IÆÜä»?(>®–"?ïçæÃãg?eÕ…ªa°?UáE¸´"?TÇ«Ss?ZR‹7¤?]xw²?ï›
V‰é<?w.¬}"`?y³ÓõÀ?pÆÖZ…?y`FþHp3?nì(Ö
«?ïèÒµ¢—?\aŠq³?ý`ÿ¬?6&õôß?g™9ås±?\8¼˜ÏÕ£AGN3FGL J1254.1-2203@rüÀ?ö@Dg_ !¸À9¶ôöºÀ;"žý†¨ü?ÖXâíþÿ-@¬ã £Îý@]€k_ʿݔûùúÇ ¿æ1Æ=³â¿ä~ùlóà¿à^¬
+AGNbcu?ï]´Þ÷? @Q)ê?ŽúÌ0çöÁ? 'í×)4?s0 'E_)?pI0B¹s4?ï3[Ao6?œ~­W¼Î?‡Ê4É!z?Ë"Ÿ%Š?‹^ûwªèi?"ià7p3?ît…(ô@?'fÓæÊä?"'¥8Çh?"t'ÿ«?œìŠ(ù£Ž?†i"\Y?ì:"¸áÞW?¡w\q´½?œfÓëòN^?"å?GY)?·%='³?Ÿ2ö6?ï\˜ºÕ5?·¨*8à2?"FP…ú?·µÀñÁ?VLõÚí¶Ï?SfR>A?ïºâ—ÂÝh?¯}ª§hL?qI£ŸóI?t¢EÂ•á?qE…}:»?w`çÓAë?ïjN½´?{Ç=ˆK?'U&éÉì?tX̯üs?ƒ\&W¾¾þ?jÌ÷(Ö?îú½­Âgæ?ƒÐÑPƒ?‡i‡ñ
½?rpµ¶
¢?"ó†TU]N?€_'n AGN3FGL J1254.1+6240@^™"ÿ‰;@K9R¿ÀtÐÀ:†T‡@сÀ<€­9‰?ً€/ÿæÄ@o5w±…?þo'ßì\?ïÛýž?µf¿»w?"e쪿â܇hGDÁ¿Öº›¡ŽªAGNbll?ïîE]à¹q?cö˜Ý5íy?V€9µ$,å?`pä.Z ?Iê	[Ú?F¹dv€"Ð?ïohê¹?–"ƒÆl¸?*72Z"õ?‹±:(au?'ûÁÙàû¾?G´Dœ?î™cP3Á?–vòᜄ?šÇÕъ?"Oú©?'ÉßGþ»?€ÉÒÅRæ?íèjýÏÏ?¥ß®wˆ]î?¢Æ 8Ä<'?Ÿæ'Ì(¶M?f_Ô}¥…?›š`ð®ôã?ïû«Á~(ê?8"ò+§0Û?.œÿ=òs?/í	£"l2?3Sv-cWF?*2B|–ü&?ïÔ>ŠnW?u÷žÑ­Ø?dõæì®|?fA'©ÚƒÀ?fˎ'Œ*Œ?nôÕ^|ô?ï\Qx!$?"ÿՊKøñ?ˆÈ2 ~?'M ‹?€Úñ¡m ˆ?pd'UŸp&?類²a³ò?ÈQ–{?zÏ7ˆqñç?o÷ÄZ(
½?qho<eAf?u)@–àºAGN3FGL J1254.5+2210@sr>À¨@U?Ô ÄÿÀ9¹âÅ\–À;ªw"^?äxg¯*"B@
¹sólÉ­?ÿî_a9€Õ¿è	
£_I¿Äò}¼Õo¿Ý­HTúÑ¿âi°IsšAGNbll?ïl±:p"?"KÖ7òš?q'йt¸?qØ؁àb$?Œ
ÉË75?'<²]ÁÄ^?ìqŽŠ¢í?ÂÌ̃É2?¡–¥b4¶?©PBæ Â?³¨<î1œ;?Á•È§Â@?íöt€Ýq?™µHå?'ÝUŒø—?ƒ¸2«2Ò?§*T	'\?–ªú.¥r?éìV4?³
þ'ÞØ?Á£·Æ'…Š?²á}D5?¯'^ðXöš?¡
þxôæû?ïΊÉ`ö?¢ý"dö†?QbGœn"œ?QÅ&a$õc?t˜(¤e¯Å?¢úÈ\Ëi?îëÜÌNÅ?®:"™L?=T€R#M? ¸öL×?"åÔ«t²?§ÎUù[Ì?ï!Å*
'?CÚMÓm?€—Ññ¹f?pÊêWø¾†?"~_Må³?Ž»Ø
Âm?íضSÓU—?"ºµIؤ?ªÓL,y;È?'´ª%´Ã·?Ž…:UÖ0?ÊgކÁ¤AGN3FGL J1254.9-4423@rùŽ?þó'@2yMŸÆ…À:[®UéAÀ; þ"ÅõB?á¦Ä'6Т@
vêb^ïÐ@Žâà_{¼¿çlXç³ê¿êÀ긽¿ÓÓàò'¿ÄvÛ">ÝûAGNbll?ïãV*üOi?m"Ï>ÀOÔ?7¾Ê	£,?>þc]–®?iÅÝI8¯|?j·ó[Ñý?ï5à£?Š(2Z8?sòêÉ¢3?u²)œdÝ?'9In|>#?‰QÕvÕ?îy<ŋÃv?'¿LL-?Œђ<)½?|dn…ùÝ?¡fÿAØ×6?i†×J)D?î‡ã%\d?šÚc™"\?m–¼ºnòð?ñdéZm?¥µ¦U?™/	ÌS?ï÷ÅÄùLe?OóÛzi
?&z_'J™V?!ÿ\÷€,·?KJTN!Ë?Mƒ…?Þ?ïÕbd›'t?vÔ
@?`;LMà¯j?c7D{Œ=¾?jbNÔ¤\–?nàœs©ö?ïd[|1Ý?€`¬ê²ý?{¡¢FýBž?pA"áÍÏ?‰j|m^?yaÏ#!kØ?ï«Z¯º1?wV'ÒZ'?gÝ8³X?jcr˜OŸ?~Ï	¨ùE•?rDÕá`:"AGN3FGL J1256.1-0547@s†_•'Í@L‡Ã¤àõÀ6'_Tú-XÀ:}Uü‹×9?üãv$˜G@ ¯X	"µ@WæÄÊ׿â[#&9"¿æ.>¦Ñ2¿åHסßZ»¿ç:àH!#AGNFSRQ?ïæžñƒv©?f™R'63?T{|j
=!?`i5<¸?^F &"Qü?]çWkºvÔ?ïŵL¹¨>?­Ú‹×°?ië^‹»/x?s]vœ¢43?p/ªªa?t%TéÀ¾?íŒä&ی?¦ÀšñO¼j?:Q¬µ?—íX—ø'ÿ?¨"»f˜…? V¢‡?ïôÂZ`§=?fãë¥g?
ä"îò~O?-¦?Ÿ¹?U¤'kA«?eó˜SI"S?ïîAcøwö?]ˆžÎýs?QÄ<q~ª ?T*ó[XÃ?Q¸ü"è?Q=w¶A.l?ïé+æôÒa?cd5H\Q?UqúŽ'²?Së±W-À?X67®DÜá?WÝ¥"þð?îA…†g8? ŒoþTT!?–žŽ¤ý?'f~£ÄÌÀ?£Ž˜—bž
?›ÂŠbå?ïý½ó–K?BøÉ÷gú>ö‡§í°Í?£7Ÿ"<?0§è«X]?B¯ˆ&ÓXAGN3FGL J1256.1-5919@røœ fè@VàºÛ^À92ÃWÙéÀ;Üæ"*¿É}Y†.-@5Í.œu—@X`d¿ËSiè½'¿éñX±¶µ£¿ßÀýFùIê¿áy³¤rAGNbcu?ìꦧt#?¶™tY•´?†ÔÍ¥¤?ˆè$'b×?¹.©îàÏ·?µ¸A"Õ°?ès-A›p?ÐO9ï:
?ž½\¸'?¡žö?¨·?Êr¨Íû1?ÍÓô&‹›?ê$;û…G?«f"Íú
<?«Y´q@×?–¥½û?À˜¦—%mo?¦i£I§±?è›Î	‰—?¨òâú¨×?£bü?vÔâ}·Á?Ì~í±HâÈ?¨°TϘ·¥?ïy¥Ín?œÜLAƒ]?pf<"çÐu?qùìÎFŠÙ?™<§? ?šæï;KUu?îÒ1»Žâ?·YÞ$Bgt?…42c^Üö?Œ×Z,aÖá?ªUÐM'(£?´q0,K@#?îËöZ‡,?•Sr\­™Å?˜7•lÊ?†ÉãîZÊ?¢gÀ–y!×?Ži-0³Ó·?ífûxB8?'T(¹A0 ?t
 ÙÞ?]¯òÛ,Ÿ?³‡z.ۏÒ?ïsÇy–AGN3FGL J1256.3-1146@s
…ߨq¤@I‰L߬£bÀ9—RMª­¾À;|ë Í¿Ÿñ|Êúç@Vô™špY?þƒ %"º¿ç³֎Ë¿Ô½Û Ø°¹¿â-ßÐúH¿ÄXPüXÅAGNbcu?ïöËTbéë?MI^—‹N?@GD5eµ?<'˜ìÛ7?D‹kdSØ|?Cs›­ú¬?︳lËҞ?€d:Šêþ?pÍ£ó ?rôkqp	B?rÙ:±?v'þ÷8V?îõGüÝ¥|?î¶…+±?…ù.qÛÏ?{‰'ÿ¹@£?–Zi3ônê?Žåá%1X?ïLn¶'	?‡ÃS"êév?^žš°Ö@?a‰=}·á?"ˆ?'ÃÑ?‡H•ðí"l?ïüî%•™b?1ýò'jC?(ٙ"ú††?'p]Šn?(D
•êÉ#?$,Ț50"?ïä;…ßtç?d…û_bã8?XÅ´]÷ÎI?TﺖÌ:?^Ã?rk3S?[wTùîX?PÄá?ƒÕ¦à'€?wû2Eu?q5É\å?ƒÙŒèÏ?¬æ¾)'?ïØ‹çÄ?c!9ܨ¶?Dә%pŸ?:l¼Î>•t?qp;Åߍç?bJÊr5AÍAGN3FGL J1256.7+5328@^I' ÿT	@OÒŸá²7À9Ñk÷Ÿß.À;'l	=–d?®÷û¸hSá@šZ]n›@ë@UZ¥¿ãì…g]‡¿êBÔíÇ]¿ä[D,L1¿ïÿåV9%CAGNbcu?ïÑaè…î?˜©Áƒ8F?:9²â>›Á?H`ð@c?uœ³ÞI	?—ÎÆAµ…?ïÊ<
?–R"DuR?ŽØF7p$?Ž
ô~Oc?‹€Š*Æ4?‹ÏÛ Ñ?îv´Â{ ?˜(ux¼?"¸s«F¶?†0ݲ< ?žòM‡??"Pm‡–-?ìe>á<E?¤¯¬¥kÞ?¦@S–ÐÈw?˜›ÙÃ]ëÌ?±µß*µoÀ? ç^Ë!?ïæMÖð ?–…ÿ³ÔÙ6?7b‹û ?VÍ:…âØ}?fÑé¹`±?•'€Ÿ¼b?︄(ò?xõØÛ3"?ršbyâ7?m…Ã	'Ãl?q#ڇkàÌ?r..êã³û?隸ï~?`ÔÉHó_?‹ˆAÿër?~uËUHÇÈ?ŽòTQÙ?ŠCY}&-?ï
KŽQo'?'Eº¹Êw?‹·ÀñÙ=ø?uq'½º²W?Ú­ÃĦ¾?}˜ÎÑ{†AGN3FGL J1256.9+3649@]×®6	@TUÀ%õ]À9 /ªèvÀ;Áڅ4?C%҄@¸'ô´@¡Ë`;)!¿Ývƒ¢êÙ±¿àÝN,çGU¿ãÇÔ©©Ì¿Ú"0žÙIˆAGNbll?ïúðBð?8M8/¦î?-hO©â³¡?$ë®.ñ˸?9ÉÉE"©?3aÅî
q?ïGÉtAŠ(?¢nˆ,¨¸?t@¤u>À5?vJÝ'D³Õ?'ö¨Uƒœ?¢!­7¦Ín?ï]ƒ‰Ã?žØoX­Š?€¥Å¨HÖ?u9uä&?‡ùX®ÞHw?zÐ-ø\WÐ?ï3A ß?uƂe2z?~±¢^Ý?xűÑ"	Ô?•Ïñzøp?·0Á.' ?ïýUáçnÂ?(Æ}ž3†?"U[W‰?ô?ßÉŠ?(LÞ@ùˆ_? ¯ïd€?ï½;rü5?'©ÀV'uó?`'¢Go?`2ڏ¯h>?yU3<[8ª?'2èOŽ?ï°Ò^ܚ?vO#ýÖÈ?r"÷ÕEã€?p´å6¸'?uÙ¼«a?i̓cqÉW?ï֑•¥Tt?iu£iªÕ2?^}8¿TT?M¼Iƒ>Ë?j/Íù¡¯Ñ?eàÐÁAGN3FGL J1258.0+6120@^`Ú¾'œ@K─U$öÀ:ÒÎX%[À<C"]È23¿êó"Q'²C@
Ì\Xp"@ÅQ *­¿ïŒ ÈÊ?Ö¥™§±_^¿Úøj
›ö|¿ÚKàZÀFAGNbll?ïÆÌLkµÓ?€» 7jî?xzOۗ6Y?€)»ï><?P~'I"Q3?Jµ¦ål<?ï§Î᭍?'óiíк?s;P{Ì9?tY&ÿ©?xÝ?2[L ?zŸGÀøE?íë§áœE?¡gB•À?¨`½ül¦? ç¦þ1^?'É¡NbÇG?€ƒyÝ¾*?ïÔ'¬Ý'?n]-7¼?\D‡tK'?Z~c3R?m*¡;ëé?hÁÚ§í›?ïÖ£%ð²?ò+Vü?rÚERñº?ÆC"b­?=B}Có­á?9¶ X:.?ïâŸê
?i²–DjI?[Šy?­??Tó/™j³?`7#YØ­»?c›Aû'÷?îz=i©"4?Ÿ'IkºÖY?£éQÞ\%Í?žËìîÿr?Ë^N½Ñ?uÏÝBѹÙ?ïù|'î±y?GþkßGd?/ þŠ?#çF¹ƒ­4?BN7ybÁ?EÓ—ÀáAGN3FGL J1258.1+3233@[±þë-
@U[íöéÀ9‡"¹À;ÄnŠ!V'À¸gÏ2f@€2t†@»ÓÿÆõ¿åsôwek¿éÂÒ¼¿¨¿âšâ™èŸ¿åL?ôŒ¯AGNfsrq?ïóEPÓ=?'³§1ñ‹?ëVÜ+<?#ø›F+?XÁfƒÁçÔ?'­
cS?ï.X¾7,?°unbH?j•ëÏnó?rOªÌ°æ?–â*ÃRC§?°1ª}.¹X?î÷¥ŽUª?"Ùü §‰T?v¥¯Ð[X\?elí#du)?›rÿ[RQ«?"ƒÊbT×õ?ïõ:ˆÖ‰?U^Šï¬Ÿ>ñÐ<]pc?†-)N?UC®•|
?UH.B·Y?ï%a'0?Àã1h,å?L𢀓"²?eDÃu€v?šwn²¡c¤?ÀÃ5½YÅÍ?ïÈË	Q?ÊÀÚÞÛ?UlpzB5?^¾Ä}q;?v?^^âèÞ?Žñ5÷X˜?ïz¹|¹?‹Ԑ8èl?h¹ÛD;²?Mó[Z?‹#*#*¨?‹8m)°?ïþheÅÑ?0®~Á­?À>ºÇeyäE>ÈeŒ^œ=(?)D¥v™?0¨MjW¾ÙAGN3FGL J1258.6-1800@sY_í¦a@FjÍØã\À8•ÜJRÀ;wU·Ây?挆`#M¯@
ÜæöC¿@'eÿ¹3=¿älŸædοæ¦(c©ü¿ä¾²¢v"c¿ê–ón¢AGNfsrq?ï÷8˜ø´Ý?MU¥yMÖ?J4ÕK:fl?H§ s¶÷?1юʏ•¤?,ã4"'©?ï­¸¿œ$?…ŠA·ÛN?r"†ŠHBå?søˆÿ?vŒ8Ë?|ԏELF?ï9ƒõ¡
?'9ߺÝ+€?‡5äç–iÉ?v;ø@Ó`¹?Ši©GÝE?v±õ¼ Q?ïˆ=çV"?†ò³°é?j‹à6¡¨¸?h®8*ˆ%?‡M—¡y?"›<í«D?ïû…î}1ë?7.O;¯?<L®ïIØ?4ÊJKèe~?-¬´ƒ°?g8g¿Ý
?ïÞ=ÆL?jTcè†^x?_ì2£­M?Y^Zöë6?aÌÑ™8è?b‰Í»3™?N™ý(?q}V­ä¼Ç?|3…¤«VÂ?gf5)Ñ?zyRïi™r?e.ìm>ê?ï熹z©?cü}Ÿ'?QA |¼Z	?Dú6"˜Ù?_±kà]TB?aQoQ¦»AGN3FGL J1258.7-2219@s£¿ø¨ô@DAMå"mÀ8®ºŸ¹À;9&º~ìo?íËùÁS-@Ÿ=⎪þ@¶?Ÿ¨&z¿ã¼²ÕÍø¿äº1"X¿çuJ%NT]¿åB!´ÊfZAGNfsrq?ïó¦ðUy?T)ïã^Pò?QFdÖªÚQ?P,C'ïBÙ?@ø›ªè5?;H(+œ?ï{z¶Kù?•n[™?|"·"ì3?ƒG"z:›?ƒßp¿~?'ލОϠ?îÿóWûêr?Š`:t½c›?r!B‹cù?Éݦt®?'H"b¬›Ë?ªØ¦â¼Õ?í·D´Ì?œbpïs™>?"k¼4ÐÌt?ˆh‹ê
s—?ªÚ
ºu
?›iæžf$P?ïøIË%,à?uIÄ~ÜÁ?E°½ãÕñÇ?p]þÕö?2P+ä;@?VŒ+2ºè¡?ïљ}ó~p?sð'Ç5i?eKæ¹Ú.?`£mó?i›Ó1?o†w–ûÊ?ï'ËÒ%ý?yE"ª§L?j—+2ç<?qîܶ^ª:?/±Pn|?kÊ鮔q?ï]öê[?€mÂ!Œe?€fX§öy{?h''3¶ëÙ?ˆ k10·?{âòðwGÇAGN3FGL J1258.7+5137@^¬Óª7@P]‡ qäÀ:±äþú2À<Й
'¡¿þz5
(¯@
¯¼{F@E$¿ÒéG¿¾²lƟ-¥¿æ1±3ÐMF¿æPöñ5Õ¿Æuyv/ÿoAGNbcu?ï՟'4©?s$—+X²ï?b3Î_†9Ì?gU¢^8>f?h,ŸHν?fžÎbÕ1}?ï¿èGýo­?~·Rj_?lWµåOގ?oC¹™Ûr?qàF?tH¦8k²Ó?î-ï°H?™ðôua? n*g¿?•Ñûý›¶?œ]í8U›Ž?†µ?&+ná?ïßµ.7÷?lÖ¼í‹#?ÔyŸJœÙ?)¸ nï¨?o´X5¶?lb}ñ˜ï0?ïòaG·?U=
‹³™Ì?BÀúõôZ?Eç»òåÄá?QÝÇ^·e?MzAªuí¦?ïéX&eM?fê$v?TÞCXv?UWÝ1ò?Xqp`àG'?`[ÄÃ/<s?ï#Ԍoö™?‰*T?Üà?ùÄl;?‡Xö^¼Z?‡›%8]d?rWô!ì4)?ïüB"ð?<ò¹Ý™óî>ݎ†È¤p`>Üñ©gáÚò?=u-WDæ?<ÕõÃ	AGN3FGL J1259.0-2310@swß (@CÓÒòäÀ9·ŸŒ¨À;€Kµàø?äôÑp@§ԖoÄ@:‰à>¿¿Ö€ºÈñÔw¿èS$Ê\&"¿µük­Ålþ¿ãM—"þ÷AGNbcu?ïÔC݋?o:´O?X1475'†?Y3B6®*\?o£ˆŽb–?i:)=eu?îÿävâŠy?¯¡@Ƴr?d¡Ë1º?Ã ˜?'Q –éà?ªUµ|ÅÜ?îìƒYÍ?ˆ#¹•"ìˆ?‰ŠEs±?w°ÏŽCµB?•û—)k£?"ÔN¨"ñ?ì"_WWÏ?¨LÙpŸ'?'}¢G\Õ?"7oðã3j?·}œ¶¸?¥¶§Ãø?ïò³|Õϼ?R˒…}§?@'ËõÎ"V?BͶ͡#ø?RW U}?Ih$¯Xú}?ï´H^5ó?€¡C¼°±?s^	*,Ã?p.yqzP‡?r}ÇÒÏ1·?w2ú^è…?©+C?yPãÄ¢g?|÷"8ºØÃ?tVûÞ¶ðÊ?_¨RÀÔ?g¦C)*0?îÈÔââì?ŒË&¨Ì?qìn-N?}×âúë~ù?–swW5­?"IÔAGN3FGL J1259.8-3749@s/hی@9$;I'À9¢Ö(–!?À;ŸÛÔ§Œ¡?ÙfJ`»@où¡A-È@îø 7­ì¿ê	‰…i%¿ßÔ«±|ÂÒ¿á&ŒÓ|X/¿Ý†ª,þ'AGNbcu?ïšá·Yaà?ŠŠ¸«,¾û?p»j©àòE?xŸLÉuÂ?€éÜå5.Ï?…Ç܏—Ë?ï<XuâÛ?¦úMÌW*5?ŒU3LÙY?"åÒv<Å?'èÊW7î?¡zë?²Ó?íÌÆ£y'š? d°«Dl
?"´óaŒ?‡L+Cþò	?¨ÙŠO˜§S?œRáãÛ?ìþ}jz? éúÀ\]?šgÇ㤘?'c…)T?±Š²"H÷?œÓNŠìF?ïæÂí®wU?m´wR‹U?PùaÕ+ñÃ?R¢~y;'ó?`ÀamÑêA?hÂ9XÓ*?ï°xCïª.?‡ÜnÑ%c?rÌϕ~S?uM7	¼JS?t÷¿I	?‰åÒÆL?ï+?Và•	?Šv4#múL?}6Vê¬?u  0÷ð?'Ùyû»ïý?‡žK¸˜Àß?ï-1ápë?'®'žÙl"?…Íî•1pŠ?r$Vl¬ÿ?Žå™R8`?|å{Ô¾‡AGN3FGL J1300.2+1416@s‡‹À]RÁ@S?ßеÀ9L#Ü~¸À;®d¾£?ÞXìd[Ž
@Œ+·ü1@×:€.Ž‰¿ê+°#"5¿ê©ó~'W0¿äïÉíÛvo¿ïùé÷¢AGNfsrq?ïû(<µ?;¥Ì䇘?4ØoÃU?2³«1ð¢?1æ_´C¼?.<îNâ€Ã?í·
dJ?±)í{ßn?¥ŠK^Re?¨íV<õD?ž
;G–Ñð? Mö5¯ló?îޞ/oH&?'ClúÛ?'aÆE1(?†UÈ*óëí?'Ë$Fª`?‡àÝQ´†?ë"è)B?¯vȗª9?¸?	µáMã?ª0FèÉañ?§3jKL? ãy''È?ïü"õŶÐ?3¦î
Jÿ?3̚hÙ:Z?+AGÛk¡?&7ló}nÄ?$[/5ê-§?ïnw¬à?¥Ãg?4ÀJ45ú?'×ë2Y'?‡²cÞÚh?''(:'l?ï=hMÇ30?"·ö"‰Åš?'oȂ?2øCA?ƒ~ì¼?xôßЛ¸?îö³ÜÍ??Š<7—/¬Í?˜w²'vÛ?")H×<ðÕ?dÑpŠ~Œ?~
?<ƒ¤rAGN3FGL J1301.6+0832@smD@lÚ@QÐGßþùÀ9D`Þg)À;¨âøˆ<z?î…У_ÚË@
ÙRl3"è@@dÊ¿àWe¿äºH«ÿ4¿æE3w•|˜¿ïÿïʆT PSRPSR?ӔtÛcq?Ì%Ùù†U?Ӂ:› ?É
ì‹e"?ØêQ$^q?ÏFÇ蝟?ТÅÇõÍw?Ó"Ÿ»³?äL³P¾£-?Óö…ù(Ë?»NZ3°º?½°Ë[Õá?âÝDo#Vû?´U;#É?̑,kK†?¯‹Þ߸¦"?ÇùÁØ'ü?°Š
Á
ð¼?Ä ›Q»Å¥?²ÆTmj'™?è³I™"©{?¸­Úé!˜?²$|Ž=ga?§ÈQà>æè?ÙléŠ7è?ÏPÊm?Ì2x£)æ-?ÃZ/òó
d?ØyÚ%iµÀ?ÎvP
Ѹ?Ûºj¡«Ù/?ÑÏ_C‡i@?ÞL'µJ?ÑWΣf¡ö?·ä
2ž?·/5ãÛð?蜶oY?®"™¹Ô¢?ÀĀ¢ý›w?¥ÕÄrT>?¹'NDÒ/?£¶Ïu"´?àMMùªs?µ²¡&c?ܸ¼
{­?¶f¿h}?§1µ>A­j?™in›£'MIXED3FGL J1302.3-3259@s;?¦Þü@=ÓÝÿú÷ƒÀ94¹šûÀ;'h§‰Fe?ý7ùÁw"@
vêªÙ2?÷…«'	?ïúŠˆÏr¿×Ð.½§¿âwõq©¿í`ö0ã PSRPSR?}éCÞK¯?ó·°Ð~È?îØtiùÖ?­6ó?Ôá?­xn‡ºM?ª0ýI¨{Æ?€g¾Ìu6?‹pï¬JÌ,?íó˜™ûzp?º§†p‹È?¬£o	h®?¹UëKSjª?«V©@;ëz?›{QY|?ê´WcÐE8?¬"¢k•?¼±ðA_à?¨©yE4›?¡š‰Eg?"­dæÚ}?íÚB[?ª)þ$_e(?®Ûâ¼	?¤E|ÕÌL`?s´h."÷I?y¾Ìj7'z?î°.®¿³?¯lù†ë÷?¢†ˆ+ññ?®ÿlõ0J?–Ýû»{*i?¦ñ"È{9?íŸÀáBa?½ºϐ²¦?±³ƒ	;;`?¸÷õ¦êøÍ?º–Çäýèp?¤sŠþU˜Ô?è§`\"´
?¯IŒˆÃ¿?ÀSý?ª•ÃLû™/?¸'m´Y%›? KéJwkž?ëWÂ-ÙÏa?§"͟?©_¸Ô׺?›oÝ´[PSR3FGL J1302.6+5748@]ÿò¾ÎÝH@M \ßÔçNÀ:…6ÍòfºÀ<$y'¼U†¿ª±›aþtP@;*Å{u@-_§°^¿ê¡:fпæÍ»
hÊÖ¿ÓØb<`-'¿Üº¯6*èAGNbcu?ïûHäSç?H¦w)ދ?:'ݱ¾CV?G/W³6/š?'"+õ³?!NÍË ?ï¬î7Mª?ˆ™ê©)û?s©>Pêö?'è•ïÚ²­?ußÆ< ð?x^| ݧ-?ï'(õ†n2?"¯=ßxdÚ?‡54#Ïç)?~ƺæ?Ž~(3?yzš«Ý?ï¼½2züv?yÑp…ªÁ?TJd•Bõ?X¡õø°üp?|ŽÍ^T–?wRg'ýj3?ïþ8Cƒã?'ñHŸ·? %IÕÜ©¸?"ò†¾Í:?²ì¨"?mlA/<$?ïåÔÉ«?d×_½ŸÇ'?X,ŒÙ~?VÐxhÎù?\+V㯹?ZbOô¨í?ï£ԕ̎?o´‡Õû‹X?u<ç|§v¡?i(ðÑÇ-?y6®Õڀ?`葴Õ؍?ïô¬GÏ«?P™Ü-¿‹.?A
ûÒ o?6:]5Ú ê?L@åud;"?Jk–¸{ú}AGN3FGL J1303.0-6312e@sÃ{á"¿Öâ:""•À8'£¥AÀ:NU\Rç.¿Ù™bìc@Æ_Ȓ€v?úDå)?ïú-Ç©­¿åhlÐ㳿â1¢4rÎ?Á!™h§^OTHERPWN?Æy9®2¿?Èp%J?†Éeí£:?•u'N—uz?éã–nۙ³?É¡ÙrçB?Ð$…†ù?-?Óf	Èux?¥҉‹j¾? Â_ß)??杰/aí?ÒâÊpã(??ѐ;å‰\?³5ævœ3?´ ¼ÿá]d?¡¬ÊDy…?䳙ÂUÇÕ?µ"Ê¿&R?ä'uøn€?ÇUIhSÑc?Pô ÏŽ‹-?^ø†©ÇÎ?×áès­‡ô?ÇXøäW?ר+Ø ër?Ó16G©{©?—åhÅ©Qy?¡fN%˜d?ãl¾Í/É?ӕ{߀ë?Ô|ðÊO?ÖAòã%Ãx?®ç´Ðß?ªéý)b¯?äъ:šÊ?Ô¿M
àúg?ÙÉ:^Ô)k?¸ç$+¢Rø?µi/ Åk†?¡zr½(ò?àn<ìoj?¸82qMgj?éKÕ²_ÊQ?¹)>ZE?DŸžô¬û?B¯ Ñö/?'
4ÞN?¹Mqü0bMIXED3FGL J1303.0+2435@uՍ@$³>@U—‹àôÀ8‰ñ…é¹À;m˜«]|?ëÒb?‡¡Â@»V†''@r±¿€3¿ØÁ'H¹Ï'¿âú¦ôÃXQ¿ãڔßÜ°+¿äNÆýTÿâAGNbll?ïùó)5Œ?EՖFÃ?///™ŸÞ?-B­Â×¥?@gÞpE?A=óP*?ï?±–î÷ø?¨u­'×9¬?j—Ù¼N™N?p۟ԖL¸?"¶Ñê—-Ç?¨A÷àæy
?ït Ç?Œëÿóγ?Ž,.Nun?…Ì€+}-?ŽÑÑÐ_?€ß7©~¯Ú?ïÙq¼Áøï?t_ù†ßn?Fá«ubg?M;eÝÓÉ!?p†ÅdJBÉ?s|§è?d?ïýǜóQ'?)ÿjòõö?!rŋiü¸?{ÓOy?"i…|ñ‹?"JxLfo?ïÕiÜñÖ?ƒhð4S_?UÔU4ï²?UþN!ež?o¬"Ê8ª?'øÄ7€?ï|ÐLLùr?ƒ%k –´?Wä>¬7?|Aw+ç?~èM'Ë?sE['÷0?ïøÿI›f?P!Ìã†?0OBäölU?+IR9QšÛ?CÜ1,DIÂ?MÉÛJiK0AGN3FGL J1303.7-4619@s~KZ@0ñ'lÀ9t.¦¸§À;ŒËÔHµ¿çƒÑ¡¦a@+‡ø[Ç@]à
Ü¿çhc'\ʗ¿ãÁöçÊÌd¿çfå\š=¿ç@>"iPAGNfsrq?ïíͲi¸ð?\8âÕ6Џ?VÂÚ ðø?TÃ4t[.•?KCö>ÿþ?L&9Ô
ù?ïsÄ®›3?•
¶]0?v/WøHñ?r×c/ûr^?ˆc\³Äš?'7qô?ï/Ñå÷|?†KÛÔ/JN?ˆ–;³bØ?y›`H¶n?'º¥g_?~ruë¢üs?îá-δl?'Á½t}?jš"'Ã?h[Î ¯t? C':Š?'ÃÓÅ]™n?ïùO~öß?DÀG£@®?Bt†%¯ý?@¶8£Øe?2$uáìÚX?1x†õy˜þ?ïÎyH]Î?{ñÃ+'G•?_ú«H+?WŽ) x¶?pÄð›v?x,HO¨sw?ïVýpa?o÷¶ã0n?vŠt?fzÿO¸ó?zì:Í ½?dB¶ø;óÇ?ïÂÖ ¤êt?kèo+H?A§8+²î'?6Õ6{Ÿ?|_ȲÌɄ?jþ©vƒAGN3FGL J1304.2-2411@s*³ S\ž@CJà€øÀ9¤0íCÀ;yIoH?ê¸-ô¸Å@¶ì²Eb
?ÿPò@¤µ×?ÕPHÌfdR¿ØIµ‹g§¯¿âAÇÝÇp¿ÚØ/ßõ&;AGNbcu?ïÛlÛ©9?dyöXdڛ?j*Z¤jÈÁ?a`}'…€†?TѓˆÃëu?IR
Èe{¹?ï&–åŠ2ô?£u{õÐ?Šý®÷6É9?–½ã[÷¥þ?‹\—°‹M¦?™½¹‹0Þ
?ÛÙýY?"'6!xk?™˜í'^i?Ã!cŽ+
?''¶ë'ðy?~µóI"?ë¬L îŒ?©‹ÙW=·B?§»ñ«ÿ? ODþŸž?¶¿¦@Œ?¥†ÆlÜ-Z?ïð$Ÿ`qÊ?TÀ©lb6P?W!ˆ³'Á?RY/e±?A*r"CÂñ?4Èz¤T<Q?ï¦Î"÷Þ?'ÑK?y\˜p?‰ª²U..?sŒ±jHÏ?}ßòöÚuØ?ïeàw­R?R'ãX?†µ:Ú¨t×?|±oSÀá?¥NoUù‰?k>Óª€i? ýY:?‹Ö5i3ïH?—ì~¨Xx?ök"ô?•ïZÍHK?ƒåMŽ1"AAGN3FGL J1304.3-5535@s^¿¨÷Û@ö© JMVÀ9xþï^ÈÀ;-QîÊN?õC5Ú£@'Øì?Ùµ@'/ÀbY¿ßðë(ò+¿ì¤¯ÿ;_¿çJÒ6C3¿ÝßQ‹Û7kAGNbcu?çÛuJb'?Æs'#h ?Á+–†®t?¿°?«ðý?¾Ñ1(Ÿ?À¿xþ¾É?ê¯u؎ç?Éj×ÿ?§ôÕ²'Ã?²Öü5ýQ?¾‰æbã?ÃlG¦Ý¤á?æùû!ÛV?­]€q°?¿dݔ	%²?¤Ò'^ªì?Äe¤°µ%L?¦s–‹ÙMË?áþê½èG@?¾:ȹþÐ?Áí@àšßë?¿¡~â*¤?ÓŠâŠ?º'<Y€-?ìö°M1®p?´ì| 9›Ø?«Êä#ÝS"?«¹
b %}?¤ÊwaÕ?©%ÁF'?í ßlÉ:?À^¨âŒÒŒ?—zÌf/?¥#ï'á¬?ª4ùOmÔ?·Ãc±êÄ?ëI‰†|Š?¥y}¼»ª?²ìá˼ h?ž™W]±Œ?²ÆÑÿXÊ?ž˜Œªþë?èçÈ2"*ç?²–سB´œ?¾–ÿBbG•?°¥xÝÒÒ¢?º*¿0×ä-?¥6V>«*AGN3FGL J1304.3-4353@s[ߏG0@2逾À8D7guZÀ:Úá& %9?ä³i0Ü@D‹çTbƒ?þ…ÜiM¿àlõÈÞE¿Ù1Ídn¶ä¿ØÕN\j C¿à'Í2|AGNbll?ïùnbֆV?BùeÅ·¿?,š¥Ðˤà?/+e]ñÓ³?CÌ5¼'$?>rô8Uí?ïF²!Xræ?¡¨¿Ì:)?€^+è¼Æˆ?}ö\-¸?õKÌ%?Ò?ž©n$«
?ïf8³I?'G¿eŸÂ?…RØ*~!Ò?ƒZ°£ìñÀ?"iÌê'Sþ?‰)8ý?ë…F¿	É5?£­þôo܏?‡
ÿb½¦?‰àÜ~¼Ž?Àz5‹µ'?£"†Ÿ€?ïüZ‹‰-?C-	mÁWÊ?'©²&2°Ù?BgôZã?1VÈɚ¶€?'"o_Q?ïºY—˜Yö?†S~'<?l™
yš?jŒæ‹md?t†­ƒcð?‡ä&‹}?ï€Êi´éE?'i''?zjE)¾?x}q¨ã[?'˜CÅã(?xÖ7¨º~)?îP'"—§&?ˆP‡,¾ü?€V§* ˜_?iô|<ß'ò?¦á,ë›o?‡SÉ ‡ïTAGN3FGL J1304.8-0338@sWÿŽÀù@M†ÿ ^¯¹À:ažõ!À;ʆ`ñ˜¿Ì$Ǟ±ÿ@1mÇXÅ@>€ vÿéìÝîœe¿Û©VÉmû9¿çñÊ8%"ì¿ÊÔ¾!¨
AGNfsrq?ïû"±f?B9V'Wu€?<»8Š·'?@<ÆV±/r?%7¸ªÙc¨? 	aµ³ª?ï¿"t‰?€ÕəJñ?mIÃ!
v?qÉßuY"?qÊ.•—?v÷g]bØÒ?ï+c¥¹/?‹uã«h?Š=]k?'ÿt ¯"*?Š§Ù†C¹?ÝZ!SH½?ïÏEç&%•?q¦ò	«?AI­ñÊ?DÒÜäЂB?v9ÃZ/8ä?q1t>…¿¥?ïýw£`Óç?2®ÐÕ°?,'æÉý¢–?0¥ÊdBA?ç¾ Š×"?Á§ó?ïè%Ñë?cÿ 2Ìþ?TÜ⟢?RuÒ@ßV-?YèÒ0HÑ
?[ƒ3W)Œ?2›w"?yí½yüö?y~ ôF®N?t<¾àm™?v6ÅÏ+›•?l×x+¼ ?ïø}	–Þ?HAmH‡	? Ä1 æn<?­"N¨ ?IÚ̙L±Š?G›L9*×AGN3FGL J1304.9-2109@s2"@lÚ@DÍ0úŒ#À:7Ϗõ«éÀ;™S ' ?ќ®Ñ(@¥í¤ܘ@.ÜÿÊÐô?ïÚbð÷4¼¿ê.f›Ñ"l¿×¼<a/Dç¿æ2rgâ¤AGNbcu?ïåêÁ"É?g:QG±ø?=¤ãU€g?>íF"ü¹?fcI¼¼¨J?eѺüÏv±?î`N‰G^[?®–e©
Œ?œ.W"ÛR?¤ IÛó¹?—ÈzWï\?¡')µ:qÜ?î+¶^C¯?–g2Ãîú?S€÷…€?€ª¢'ÀR?¥Ù¥APT?"ÉTgùH?çÌȐR.?¸"`šºúê?°†>­k±Ê?¦ñŞ'ú/?ȉ¾g%Ëc?µ‡Ì–rÒî?ïögq9T?Q†GáË¡?/ax·qܜ?2¦«a.
?N‰Ýìä<?O»_0e]?ïXœžS4'? l–m†õ?‰`L-ñy?›vxGÞg´?€xŒ71L?‡šN
Õ?ï5ÜêÀí_?…@¸L¥.ª?uEåÜû?rñ¬\E??‰¿¸»hŽ?'k$	vV?íDèNªÕN?žp–Ú¼=?¢©˜Ì?Žß•›@	q?©j–M"?˜}î§ÄÓÐAGN3FGL J1305.4-4926@srÿÑÜ×@*¿?>Ú0cÀ9 ×{|xÀ;jmH÷Q¿âU©´]®÷@)ê'/—ó@j`_'5¿å²À²W¿çXÞ=¿âÆì]¶¿o¿ãõç]qËOTHERsbg?ïá۟"?e¯9ʽs?a°GnÓ?[ö!4«¿?Xè»^Š?[â6ÖªÀä?ïiO<±¿´? Nî?y枖>×g?€­€qv…-?ˆ¸á™ž³E?šñk¬e?î†XË.xJ?"q±)J•?"gwgÓim?"òŽávÎ?›Ío0¥¿a?Œ*ÎɈv?íƌºÊ'?ž	g
dÙ?ue
fiP?p†É[FÙH?°uIR£HÁ?œ¾2³º	Ú?ïöc©ÈÓ?Kö^ŒÝÌÒ?IŽ|t=?F2ςÇyü?9Ư
X}ê?5œ]p…?ïÀ!±^9û?‡ú¥I¼fÂ?e¹e3¯Þ–?gÙ¿…Û±u?ut¤}/y?ƒOQ+S±Q?ï]C•+é?…RÆŒ@ì?'Šow_œ™?x;>‰ñb†?†$«AH?{}»­˜¼"?ïwÞíFûù?yÿbG2?Tö57'	?DtÍWšD\?i~Úق?yWC&ÓûÖAGN3FGL J1305.5+7854@^"‡aˆ±@Cæ@;YrÀ:	!0Ò/ãÀ<¥šXÜ:¿ï¶ö˜'ö|@
Û'òã6ò@ߚ¯Ä¿à¤kTôÏ¿å€ÚUÌ¿æ+ö8+¬¿ã™{!ð{åAGNbll?îËç»vÊH?¨W<ñ°®t?•«쑚?¡f¯«a"±?×y©Ác?—='¼ÑD?ïD¾À'ø]?¡ÇK™Ÿý?†!‰iU"?'r wÒq?ˆ®Æy
™?˜z·Kô/?ícWqš¼?Ÿé-6·$¯?£Qm
K?—^0Ïæ
º?¦~—xû?'<U×ß
Î?ï9Z™T?•è`$x?wsmÈîa?w•'QFã?™;ðÙâØÿ?'ÿhðM²?ïÞm'ÄW!?t¬kèà:?Wõ½óŠ?`eK¬?e—ŽµŽt?poü`dú?ïÏ#4ž©_?xrtì¯ùÕ?g²ïJ?jÓر¾É?iÅK†‹©Ó?p—u…ó´j?ïB™F|U?‡>GõsEX?ŽL§£r‹c?'`íþ?Œ¢²
î_]?tR1»bæÛ?ïÜé™BS?l@÷Al"?C‰JV߄³??n??n4ŸËX?j´ÂjJXAGN3FGL J1305.7-6241@s	&ÿ}ú?ÁúŠ ,…ÅÀ80·omv%À:E\jd!é?㳐Núu@r¤@;¯@΂ÿú Ã?ïüÙ9™m¿âó^œm‰p¿ßÊ'Áe¤¿æÃx;%OTHERsnr?²è,	—Z/?³"ZH²´?• 
ðHç?–ͳ-'«?ìùúƒ´3?¶ÏläT´Õ?²E%UegW?½Ju€Eñ¸?»&0Û
:?·‹¸»Šê†?êR•9ɶ~?Å.ÒGØS?Ér;ôDWj?²«WÚ
Â?¸ÌÊ0€Êl?¦¯8#sQÐ?æ‰×¼ŒZ8?µü=É¿E3?Í»Ií‰Û¶?¹y$嗽Ú?©ÀEpp­?ŸðpeϯÚ?æõ)-±û!?¼GoßXb?Æ#+ÏÍÄU?ÃLƒfQm±?'-×1]MÂ?'µȓýÚ?éíÆRÆ\¬?Ä6
"Ò~?ÂK_FX÷4?ǔ±L¥
?À¯÷&ñ(?³kL•[§?çA*d­~©?Ë]Wôޏ?ӌdd%ü?·íÞrÔ?¶Û·åù³O?¢	Ÿèu¸?ã^VÑ.A˜?¶WÜCüóË?ֆčÁ§³?ºÎ¤N–G?ª?I!Ëa?–+¤Þ,Y?ã©'3Ô!?»E"é›(OTHER3FGL J1306.8-2146@s:É?¯Bx@Dyá`xÀ:I9¸ˆr*À;•"ô έ?Ô¸>Ã5@¨ÇÄû@@,Qy‡Ö¿æùx`}²ø¿Ü÷q¾*À¿á¿°ÁË´@¿åÌÔ^çl
AGNbcu?ïäHnG ?iòï(×L?QØßÉ?K"Š1ëpÊ?c´Å'nt?eëdÙC¶¸?îÞ~âvZ?¤P…uí\?"'¹»=Ö?›ô`‹Å–?j·ÍÄì?—mð:¾€?îš+ò?Ê–ü½H?ÜɎÃn?€"ËÙò¢?›ßÒïî¾N?"zÁè@9?ëÙ×Íy?§Ø8ñÑ"¤?©Ò±ÉSU?œA¦'ÅR?¶—Ødµ«+?¡Ïoƒ@$?ï÷n
Ï¡h?LÀõ+룐?5M£4äm?4µVu8!¹?G ÷¥î?G‡¬éBš?ï¡ìÂi$9?‰UÆê?w™D"DG?€!©7ç5û?wpZÌxjÕ?~‹~©¨ê?ïg³ÛÂ?{þ'XåY?€¦"ììˆ?vÑGU^<?…l"`íî•?k\âØ~?îqaä÷eþ?Š«2Àã?›ûôþPE?ä4cÛW?–¿Çlð
?'RS_¨AGN3FGL J1307.6-4300@s!] l‡@3Ň?úÁÓÀ8yÜ>Y×ãÀ:øž0Ø ¿Ö3ãVüæñ@A×*É­3?ýf	AGH¿ÄNñTÁx¿áæF!'9¿Óôõ~"¿×´]a§\AGNbcu?ïÛÈo3Ù:?j™è¬£ÍÕ?PMHŠ–È?KÕÁ86b?l쪗Q™?gJÄõ=l?ï‹T
ÉA?•ï' ¯Œ›?v›¸´5°?ƒ![0q?ò"×8è?'ãɌ¨#Þ?îø†"?ŸuM#×	?«4¦?"Ì"Õ¸´?§,3yOd?›g>¡¨=?ì4ƒ75?¢.×¾i?`'g±øÃ?\åÊ£‹Ÿ?½Ú´î–?¡ûh[Rù?ïìõ°µƒÊ?`>ûîq"?Eí:í¶p"?F\In"ùã?[£~Ñ?ZzÆpke½?ïÓUñŠW˜?x׫±å¸?ap&Œåä?\‰ëyQÐ?k:pÁp?süSÃ	¡2?ïûwkW£?¼tZ²ãt?"Hú9~f6?{NÓÐ\±T?'\ö-΂?‡Õ.eÜb?îƍDiM?ƒùÄÒZ?R–aš"ƒo?B äñ5'?£|¾è?ƒí\Â×36AGN3FGL J1308.1-6707@sþÀ//˜À4›ÀzÀ8kË^7üÀ;ȯ0ړ¿çÒ:"T'@"ÿŸ‡ð@™ÿ…Vl¿ä…H=JR"¿ç_ωÿ¿æf  Øxä¿år›ÞàæAGNbcu?ïàm¿‡P'?l	k¥b?HÞ¯_ÍØ?PŸ!•j?iZ"ÞåLL?iÚtáÄx?î7wªJ?³u~wÎD?ƒ7¬*ÊÏ?ˆ€
]nI?ªèA|´÷è?±XrS‡?퉆²ÈO÷?Ÿ9Z"¡U?›eÊ-aíC?Œ·ÿâÙ˜?©´¯¼Ê	õ?—ƒ9ØT?îÏòǐÖZ?"«88y?EgåN4c?JÉZÉǁ+?¢«3ô?"ˆÝi(¶?ïõ¾ŸÎ-?LLâuòä?6ô¸ê´ê?5Â@°gÏÄ?M‹'R¦Æ?GM‰·,e?ïHX©ê?íð	È?oì¾VªÃ ?s/v}œKB?'÷SAXú?™×Kó÷ȟ?ï#Ñä8Ï)?†®á‹h?†b.ߖœó?y´q=Ý>¶?T¬ób_?~Løý?ï´Z†øñÞ?q«
;Û7?$"gZÕñ?'FwD?'—+<Eã?q"òqÿyAGN3FGL J1308.7+3545@Y8¬À½ÊÑ@T'Zà f¨À9®"ƒ‡ß]À;߅¨K
E?×ôNšÜ~Š@zŠô[é@ÚD€"
¿âŸ ®1'¿ä°ýëü¿äNdíÈùa¿ì´@d|´åAGNfsrq?ïÚ:Ê	¸?s§o~?p" V?rÒõãøߏ?F·ü~¥c?Ajß»OsN?ïP²"´¤Ú?¡úr]¦µr?qŒøðÅç?qÄÓ%KÔî?'¦Š)oB?¡gFš ?î[x»ll?Ÿª ±m¤2?Ÿ">WúI?ŽñÁ5\1? =·R‰‡?™]#‡ôŸ‡?ïºR«b]²?~JÅ6ݍ?gÒd³S??gmDu|?víxJ?yšc
ú?ïæ±UU¥'?|‡Hø"#?eð¼¹ÙÓå?ylêj"°ð?:ïo?J¾n¦'"<?ï½ÝÖµXè?=‡òh—ã?\' Ïé?\lQšKû?y쌾¾cø?Žâ_³N4?"ÚÎK?˜}VÄ?"ÁeR¤™{?‡{ Ð¾ ™?"H*"e3?"ƒ(þvÉþ?ïóC5"»[?WãI'¬?IÙˆÅL¿?B¤PB+BÅ?Igÿ8?Tdí¶k}MAGN3FGL J1309.3+4304@[Έ~¿"À@Ri*ùš‹À8¤D¡À›À;Cä1m`V¿÷¥Ýað_ú@±«3J?þù_Js¿äBûxdsP¿Ù|ÙW¿׾íñµn¿ä ËR+úbAGNbll?ïëRFÒU?^z›ý«?Q;v,eçK?K©È˜…I°?Xü<®‰y?T† @CfX?ï 1E>ÅÛ?‡ûæðÙTA?s‡Î¥ð"?un®Žê-L?|_Ž§–f?çC=
õ?îµÞ1µ?ù?"|M®^£?Š±™è	n]?€Ä–¢å6í?›ëlÐ+ß©?vӇV?
?î¨6Í>=?š¶ÑU®Ä?dR¿øvqh?t~ٖ^!±?¤7g(
éœ?™®@AOê?ïøPÕõ.Z?E!©Èsx?<Ë{6'Ó?4äÿj'Œ ?@VêÓM~Ù?;<ùÛ­}í?ïÞø°Q¤?j\LTµ?]]XúVŽ?[8»yèu1?bX£ºÈi?aŽdñî?ï`…4n÷?''Ä|?€"ô'à§?uÀMª±.?‡Y¾Ñü%o?z-ÆCê
A?ï¥ÒóW{?V8àâÿw?6{SœU>?A",ó¨ál?†2›Û(µ?>äi'*AGN3FGL J1309.5+1154@söÍÀÓg@RŒ "µ7À9¿þÆDÀ;®ÛÇ4Ý?ߌð;Å[@¶EF0@%6€o§?î2†wÓÌ¿äp®·h•¿Ô
Û«X*¿ë®Ž
ÒÚAGNbll?ï'Š¶c?˜ÝCi@žF?™.PˆI3Q?— ÆTP?w³/·¼'	?r3Pã;ý?ê'áìÎ(?Ä'JÅ~­c?¾Û¶è'ƒ®?ÀqbaI?ª€péý(?®¶Ùܯâ¿?ëŽBj€ê?¦·Usþ>/?¸#¬,™;%?¢ì0Ê?¦Ô€ü7ö?"y´9l?çÎn«F?»)qt?Ãsи¥ß‰?¶PvÒÅ4?º¤í±ZÔ?±¹%_ÿÒ°?l÷á4?ƒ6—÷ï€?'ì¼òQ?VmÐ?f¦ŸP§å?`¾1ˆ?í`V¼|Ú?¹G³¨Ž	?®UòÅñ?¶Ó"°œ?—K*_tæ¤?û§`¬~?í¡í{$9?ŸÀ£¾ªŠ?ª
ّ¿ 5?™¾jYF5?—¦tUÎz?Ý'"ôúþ?íTsóu`³?Ÿ¶¿à#m?®˜g¯*"B?˜Ð]êp|?˜@²8&+?'cËöEé…AGN3FGL J1310.2-1159@sc@@IOjNÚYÀ:4Þ]	À;§£3vO?Á"Ç<6‰v@
Ãvõ׈?üÂÀ¿xPt¿èãeJ\š‹¿Ð|û3ßοæÒYÏ:w?Ѥ\&'²AGNbll?ïàK¡¶k?j2¢"5?MpŒ®y*c?F9€C¬æÒ?hX;«…´?gö]üG×5?ﯪø1I?ˆMêãpúª?rlkÙ¯î¢?€Ro$¥¥?u¾-æ«?{Ô_‰A£Š?îÇýD¹Ã[?‹žb<­Ç?ŽZk"Gž?~^¦<™?—Ó!¢'ŒÖ?ƒ:9$ä?ïWÁ˜W'?ŽbA"'ï?d§ý³h-?r|Ÿ˜v+?'rÍLÛm'?kÑSÇ?ïõþE&?P¨Î\n;Ú?7ÏZÅ.d?8ð¶
Íý?L='"tT?IŒUÄgÂ?ïà%ª?€Ù›tªí?]c}:Ù¾Ï?v îÊéìÅ?`±&<Ðvî?iÔRôë?ïhðëvAa?x¦/ ¡W ?›ó³båË?qb£ OÝ?"'Ñ^Ž¢?júA;"ï¦?ïâJwóV¤?f19󾖐?B¯Ž«ž×?J;Õp˜Å?i	¤"BwÚ?dN6Sn@AGN3FGL J1310.6+2446@­öàF§.@UFãåîÀ:¯3‡	WÀ;à_?³UX²Â·*@
U¡¶ž@jÿ¨AR¿è´ Â>¿é)"R#J¿Ý)nÛ¢J¿é¸ÞصZ¸AGNbcu?î‰#o›ÄA?±?ût~M?l˜™ýâ*l?p‰£jCcÚ?¥¤?gƒxÄ?°¨%û‰›?íà{ÉáJ?Áâ陷!?‰?]â)‹?"€å4ûôÓ?«¨kç¬7†?Á=ę^?ì´0ÌÚj?ªBGo¢œš?˜—V"#?Šdñ²~?´8¤D¨?¨£H´l?îIsD¬h?æÃù&'?•ô¯/|9?'¶$ޔr? ntŸ'n?"vH9º?ït#Õa	Ê?ªš$ft{?døèuú?{žJPÙ©?¸Ðt)Ñ?¨ýpɑ?&)NG?Ÿ¹ƒÿ/s×?p-óC\2Ê?s&"''?‡?üÝEFÚ?žÓÅõ…?bPÆÜ?—цÑÞ?"ïâe5Dù?v"ÈéÜ.Â? šB'(?–¯]"àÁ?ïƒôá¦è?xB‹ÁÅ×Ã?ƒlø©þ?n÷\%™dd?wÙ'Ê[Ò?nã÷V#POAGN3FGL J1310.6+3222@Ugáßîè@TÓ¤à¹)À8éqHA¸À;2ªýo?ô6°x®<"@IG¨¶)@8ž_&+8¿âr<Í)®¿ã`=þúW±¿äjg="¿èºùŽ‡ÿAGNfsrq?ïòÇǙ ?VÄ"€ƒ$?Cö€V¹q?DW~;êŠ9?Pu0»­d?Qkkaa"§?ïQH nú#?¤°ø¥«'7?m'YžŸÅZ?tu$Æ9?'$ÐÃ6ý?¤G5Nºyî?îýOú©?'±;ŽÝ?³xgðª"?‰™'ºa£$?EIn«»?†‰Moj34?ïÈ¥8'Êv?zå½ª÷?XTT w?at×Çà?u˜N˜üÕ?x£Ûæ¿íä?ïö»Ö…]M?TuÅ˙ûx?FŸêr›'^?J´¹É_›?<áx¡šî?I(NEOª?ïÉpj‡n…?‡í{ѯ ?X±n´SU?XmZjƒx?uoEø?†È×bÛ?ï[í^	B?…}¢Ñô?†	§uY±=?#Óñ¡ñ?'ûý®ÿv?wP£Ñ¯ù?ïóZ†=?YÝ«‡!Û¿?D>e&}?D"ósù?Nw¨øßw%?U÷¤H=–BAGN3FGL J1310.7+5515@]I^_0çÿ@NÓ# 8ÜÀ:V÷~0ˆÀ<
 Òrÿ¿ó&—ºo@¿ênô)ˆ@7»Ñ+¬¿èi>Tpè¿é¯"4LZC¿åjY­"¿ÖÅZ¡¥ñ[AGNfsrq?ïþ5ÇÚl?2~ïU­?=·mÁÊï?%'óZ
`?!¢šÎ?$:Ðj9?ï½;ÓHoŽ?€¿7Ñ9+b?mXwVøÜ?r{NòUÄ??rµÚ"Îë?v ê­õ§{?ïGmqtÂ?…|f•Ñ²?‡KU%ç¿C?ƒÈ82Šb?†ÙN‰| M?q Öâ¹$?ïð´&ôÈ?]Ì&
fB?8-vÃJ?íd‹ƒV?^ìÖF
æ?]Šd)ðžI?ïÿlˆÙÔ?£,{ïÎ>ùÏ㌂…?ð?å4ƒ½?öPm-iµ?øãjK§?ïérŸQ5õ?cû
Jï?T †'q?R»Æ݋s?Y Œ¾óþ?["Z.ßæT?醴tÿd?vÌÕÛe(:?w¼#³î—h?v íz06˜?tè!Ãpkò?YF@‰œ¶?ïþAý"a?0ãÓL>áp0Üâó>Ýò`TïõÍ?*É#±Ë=¥?0µÆ¹¼AGN3FGL J1311.0+0036@sB¡ Ï@Oˆ×ÀEÕÍÀ:¦.fDØwÀ;­À8iÓÙ?›j)?@vwY}Ë?ø¹€C‡>?î7¡Zî¿Ð
µ|Æq‹¿îw}»þ¯"?í0ÿ1#
¡AGNbll?ît'S+öÿ?°õ£&Àq?œKQ
îèò?£œ(©½4F?•$dŒ'74?ª€Ï%ör?ﳓ†Á5ü?"ϽÀìú?p¸™oÃSr?u-N‹_	r?u}£³ò¯?~¢k'QÙ2?êóA—5Ly?¨ƒ'Ã6¢´?¸u¾š›Q?£ÑÅ;%Hy?°c}‡»å?šñÛ
Óm?íùäLg¯?µ=d›Yr?"2ºT‰ ü?®øòùòñ?¦È^Óóû?®ùUsHy?ïPyÛkԘ?™y¤p8Ö?ˆð7Ânz?"7Ó937?'ñQ^:÷Ž?ŠÊ&˜?ïãêáa¸?iÑha!]?Y^8¹Æ¿?^Ј99"‡?^Í¡"ªén?_R$¦W·?ìä;ÈûSj?¡"Ï¸™Í?®Èâä9›š?g¿¤<­'?¢ó`ŠY_Ã?'á¥MÏ<?ï¬]Øî?—˜±,d?rÝÞÅV6?"·L)S?vó›!æn?"¬n<ÜoÑAGN3FGL J1311.8-3430@s;0À&Ì@<.Bßx üÀ7vßY—KÀ:þ™‰©aŽ@ŸêŸñw|@ª1ëàcX@Yèb|¿ß\-WÑù¿â`ЛŸ"l¿æ!±U¢ô·¿ì?@]EÞåPSRPSR?‡õށ?‡ã­‹T¾?ï"‡'Ú3?ŒÖ‰ˆ+<'?oz¡nh«?uávßþ«^?yï^PÒQ?‰Ü
ðI!ß?î$¹Æ"Ue?¸ñ=¤K/q?ªvwÐwûZ?¸Qy¹¥3É?ÄÙNÕa?¬¤œUÿ!?èÞÕäߤQ?°9PÚÖ(U?±žÎ­d·?š÷©Ï"¨•?Š1^üø&?ƒ-œ‡»å?î"à«Á?¤+þ›"‰?§úvã"+?¡âÜïÙS?Žƒ"rÞÜÔ?"ý<þö³?ïWñxJ5ü?—}ÀŽê­Í?w…àƒ?A™¬Ô©Ï?ˆ§ÃƒG?"ÊôLÆì´?íØä©s'…?¹EmK^­r?¬Gĉ¹%?·=DXDp»?Ë}ãÈ3Wh?®0ÿí¯?çP…vvÿ¼?±SÎuæ®m?­xž¤?œlq8§.?¡—°AYo?yCJь?í¥q÷g¢?Ÿ¤ÿÔ6"§?¤ëÒÛáf?–Þ"öFôPSR3FGL J1312.5-2155@sVŸ¶M@DV}€^_1À8¢kË*5^À;9ÜO σ?ñlP5L"@Ž©-
z,@™#@¡Û²¿Ý©á§òš3¿ÝŸ^Ï('¿á¯ýã¿ç:ˆ»ê–%AGNbll?ïF#|ÿ&‰?"ç%×/E?Ž¹5½½jx?Žö
كܜ?{Ö
´?}Ój"ü/"?êËáb[ø?¼,݇ôÅS?¼qѲrk?·fò|"–ð?ª^Fyw¨?«†P®Ç'Ì?ím£k¡Ü?¤
é!(Û?¥5Œßäæü?™É'hß}?£ð<e!r
?—(x3ad?ã$ýæJL?­¤®=Éè?ͬUë¼H"?­öƒËH¹?ÆGªŽ<?ªe£~›?ïÃ0Hsó?|d]E(Ï?u eïÕ±¿?v#¼Ëµd?a'ñý±?aŽuM-á?íÐIÆÑ?¯q#ÑèÖÉ?§†C¾L«?©÷'¹?–ñ.:ÚV?›ý{µ:Ü`?ïó›:6?'LíÙÍí?'?¶ÿO
×?ˆ"û/"JÙ?‹Ãˤâ*¶?'ÜÏ»ÏÍ?é"
uœ1?šc£Z»÷ã?ÁªBÁ%ê?•ÐZ	±£?°Ò(w©?"™ûÆ×RAGN3FGL J1312.7+4828@\We^(ªC@QiÿãzŽÀ7Ägˆ¥UÀ;ýG¾Ûs?ð¾Eہpƒ@ lf*"Š@Y?ñ½ß¿Þ.3>ƺ9¿ãØ:Ö.#¿áNÊwvÈο䝞ö>¤ðAGNagn?ïúÿ	Wd?D°`;gtý?!V?ž€aµ? pÊ°ôÔ??\"4º}?BØ7¹º8ï?ïÈ]ЦÝ5?}ň,VA£?g™¦Ýƒ0?n¨õ¥†©Q?pD_¹Ïž?sÞ+/Ρ?ïRaØüÊ°?ˆû¶~~?€<G—¤?ws(¶–vB?‹+B>A?"[›ð«‹?ïþfTó¢O?;S²­¨™±>Ê«ðq*'Û>ø,•yQ©?)/üþàôŒ?;DÞiŸÜJ?ïý€½ïS#?,V'
£yÏ?ñ±+±?µóÊã{?)p§.¼$?'J=CD™c?ïèÊdÍ]?l"´b®-?T\e³Bu?Um§òJ?ZÑÜ+'‹?d»Ù$Àôè?ï‹õ³¨Ä?€«€ŽIö?y½k§ä )?sºÅ®‹qJ?€#ÝQºí?wâŸÓT?ïÿØÊ©Sm?
Â<dÍj>¨ü'BŽ™ì>»«]e«»>òÒ׺!&?
ŠE>«ÅAGN3FGL J1312.7+0051@s­›6†¥@Ožm?ž{À8Óî{s=åÀ;‰Oçžà*?ÿˆ¦½@°z‰^
'@öp
Y.ð¿Þ¤ÍÔJð¿Úï}XgÂ~¿ç¢o-Ô¿í9"Paí0PSRPSR?wfn2[q"?v(OŠÅÖå?ï´Q«Ä>‰?€QfãÅÕ?láxÄ·?qFfÈ2GŸ?®"6šGž¸?Á'™KIÕ?ëš=IrËá?ËܞV5Ó?´úhýŸœ?¿`ؙþ?¾ŸVqüœž?§–c}TžÑ?ê¤Ptë?ªÍIŒu?¨|KÎ1<=?"°LoŒƒE?žkhržò¹?©­+p?îU"¨Çg'?šk">95Q?–â"{SS&?Ògáþœ¯?e
9c0Z?h3¡™Íƒò?ïځ&—T¬?q˜4Âiù?`tŸ¯ËC½?_ê$OX?½•"UŠ?Ì^-E;&$?龋è]?Ð鶥̋g?´v~¯¯ñÐ?·rk<XÈ?Æ$ºg£?© ]âlí?é-''¥–?ªnh£¹u[?¦JCä–?"ãQ.×êô?¹0dz<¬æ? zFê‹~Ã?ìNÄâÙº­?¡r-âï×q?'eѺ(È?†9APh‰hPSR3FGL J1312.7-2349@sS6@c^@Cdó=<¡À9£úoFÍÀ;gXv¹šÁ¿î6÷'`¹v@tÎ0?üÒX_g™—¿éS''Õ¿à"ú Å‡ß¿à1oóœ´?²¯'ÓÉ/AGNbcu?ïõüMN?H}?…âí?=p=lò?3—4­©±?IV«	<•?Cóʁ'—w?ï¾5
÷?€lրGh•?h¡ÎE«Œ?j2:ÀëJ?t"'0µ"¹?xîœRøõœ?ïIrÝÜÙ?N—	íϲ?1ýþ?q̝Ž"b?ŒŠ'5ieÂ?w+ $X?﮽ëæöø?z
iƀ'?%É»	h©?`|A³Ù?"2_-
…?z5èº×?ïü·ÓÓŠ?/ªÅå½?'f-rû? ,YðwNÿ?-ºDÝìY?''r¿í-?ïç'Æõ%?g3%Ә}Ä?U7ñô" ð?R¡—Kt,?[¢€ÖÉ?aoÂ÷\%™?ïªÃ4r£?k¸]†›Hœ?rQÞeº÷?\b&$Ô¹?xŸ@W M?d®(ƒÂÞ?ïð³[Y†?Pµ».Xõ>õ&àARÀ>ô†¼Ýޔb?^D®6X?P{Ç?§Ý@AGN3FGL J1312.8-0424@s'#ÿï9@Mé_ªŠƒÀ8ü2Q‹ãÎÀ;"ˆTÍ·®?ßý»Õ"Ù@Ø´ž­ªž@åÏ_¤*l¿âvÂé—U¿çRhÉþÅ¿ç Q¾+¿äâ!…U<AGNfsrq?ïýDn™æ›?,œâÕ=#
? ηë{s?¸n†®œ?*êZMÇo†?%Þ;AvÙ?ïĊjôâã?|õ«èπg?i{ò|¥;:?m7YL¾DØ?püÑ^™HÕ?t`[-¤Þ.?ïQ™>B)?}oËT¨©ý?}Ð"¸Ü»?gD*""v?Œ±£Bé`?wÏ>"¬Ê?ïìMº.JÒ?iôA`™¨?$oÓ[x?0Îf›†Ï ?bkT‡¢¾_?ib{@¯Dì?ïþâªý?d*Ðҍ5?´À˜T ?êUw"{?åiã?
[ÃÈ?œ
?ïéÞÚQ¬?d	2Pƒª?T'Ó¾4ÙÓ?Rùз ;×?Y<n¾¢.=?[ýd¼?﫼œpR?l4Ëû§?q›#½ï?côþ|?¿$?x†ÙG·S.?a§¨‰Eº?ïý{xúÆ?A^Óyö"?	ïùŖ·¤?¡¸«Í;Å?3Æ%¸V?@ã€/Ÿ±µAGN3FGL J1314.7-4237@s7üÀz®ó@4	›€#¦ÎÀ:Edè·äÞÀ;Ø
°÷?Î=ÊïZžæ@u!àO‹"@¨_–¾s¿çš»…Û)e¿Ý‰áT2 (¿êß¹Yí¿ÙaÆ¡´AGNbcu?ïã²a¼ˆ‡?mÇϝ<l?aˆ'p–+?hÕ°â½¥??UŠÉ%µ‰?T\Na°?ï[ èá^? °÷#…P?{d~Ÿå-'?_ËΒM4?‹…†nÿŽ?œqî!3Àó?î¹VjgI]?'B}Ð?"ßçæìy?‡Êkõ|?"¿RΟƒë?ÑŒl
óU?íÎá¿Î¼?Ÿ0{¬`Ö?‹'Ñiij±?ŒKP‰¥óª?¬-/«AÌN?šêé=QâN?ï÷{×¼¿ä?Oá:вö½?A…:aOôS?G÷lGq™?@‹gMÞ	\?:–—ç&è?ïÎ6x{Ö?~_-‡¤ê?cÊ#šyìh?d€]pã?mÿd&(´X?wZÌýWž?ïXø«¼ Ÿ?ƒ3<{"þQ?†	´^Á×P?{OÐL‡
×?ƒ¸ ½Ä¬ý?s¡^q"ØÈ?ïyåpÿéÒ?¤«HS8?rˆ©W2Þþ?eÃkz!"4?ˆBO
Œä?zþ€£6YAGN3FGL J1314.8+2349@½Ðÿ·ZË@Tñ9èîlÀ8ß½×fƒÃÀ;ltK+w}?å±n Ø¹P@à÷Gʙí@b,?¤Ø¿Ññ¨Ys¿ß¥!¢'¹¿áÕЪä¿á§ÊlÓÆoAGNbll?ïÚ"'êw?n<ê Ý«?b`¼fK?]	{ô¬?cˆÎà–4ã?eLÇ^nåW?ì¥3Š_ٞ?Ãú'æWjÿ? «YEÒ®I?±²¾}°ƒ6?²€·a¶h?ÁxL€>Ý>?î_'²« ?˜—øbZpÂ?–œ\ë´»?Ùa¸|Š?€pچêX?÷[ŽŸ6?èo™¬þ•?³IOÒ(Àä?ÀE-]Ӓ0?±yÜ?»ø×Üd3J?©Ù€¯$á°?ïó±IÓM?U¨ñ⅛?Läxåc"?D–¼ÎÍ?GÝVU‹#?NÏÑ3/6þ?îù–'…fB?¯Ç?‰Ìª»?ŒÆù2¸7_?¢¾¦.Øz?'i¾u÷?¦ã$ʝ¦?ï?ŒR3S"?‡Ÿ²9çs?ˆ•ŒG5D?€è·»¢ëÃ?ˆUܕ¬?|^ˆ=îÑ?í¨¯Ý¹ë/?•Ö tÏì¯?¦úi¢…ü?‹ë-?f7æ?œõÇ|\Æ?+X¶^þAGN3FGL J1315.1-5329@s(`ÐÕ@"p'`@3À8Π°P%À;7€ KÏâ?ú¤Q›©@C¼«Âf@}KCuJ°¿áS-ë[êH¿æî¸É÷¹¿ê£Ó€‰ìí¿ïþ[2*ʄAGNbcu?îý¡6ؐ?™ìµxÜÛo?"^¥mF?•†Ó£5?‡Û€ÿم?†­Y¿äÜä?ë6&=è?Á"|q?³I?¬É"ùŠœ?ªN1èÿ_?¹qŒQøê9?¼Çgâ)?ê6Fš\üÊ?°Œ5ö9u?¼§Åz¤6?ªØÀ– ¥?±¦,uz?¡¶‹ôä?çöÍò¨m?¶ÃsO‹?Ã0Sãƨ?µ*wYsÍ?¹énX£/E?ªÔ0½cØ?Θ¥?•Í—¨Ë4?‡± ³y ?(€Üò$n?o¬®SúÐÚ?zp*È?œ?í=OŠñyï?³ä£TÄ®?¢ºQnÎ
?¢LmŠÕ®?©pöüåÞ?«•åz?ëºÖò"[3?ªÞ˜d*ðñ?¶[¯<
åU?£#"¾Df?§›2aVP'?´gr¢VN?ì)%h34?¢Ë®—<#?¶óxnÏâ?Ÿ¹Ì6qM˜?Ÿ¹™qß?"§{Ì­ÔAGN3FGL J1315.4+1130@t?'Àa"@RYg 5)­À:'ýýûCÀ;×íÂæ™ý¿ÃªM›œÝ@+A҈M—?ÿdï`u‹¿íYo7¿áXwŒÒ½¿ßW.e3?Á?jƒ×e'AGNbcu?ïüF䄾/?5?ìöT,í?(X4¥Œ¥?'À4"ö±·?1œÁ'âN?*sI€àÄ?ï¿(šM?'^V'û?nKbû]?x¨¤í"Q^?qFB(ÌVu?tsü3'2®?ïW˜hþ,|?}B<"?€óF	Tâ?r½ôÏßÄ?‰&Ÿªiph?s+dJíåý?ïÑvVbQ?rŠ."d'?5`ÔÑ«2†?I–L#1×?uîǚE'ˆ?r/òԋÅ?ïºí"‡?µõï¿Úº»?t쌙J¦,?ª~ä›ýJd?k9ÄѼ"Û?¡ÊËå£Ê?ïç»4ÁJ/?fêQF?|?T²hဏ
?SÝÉ8á{?[×-3vóO?`è4ëBÑZ?ï©~°xòõ?j½¦ÆS8?r(Áä•,)?[ö¹è"š?yåÀ´ÉŸ?cÞû`!•‰?ïù½×f"?FM…@0?òaž? Y"ԝ°Å?HHø8(Äÿ?D³>';AGN3FGL J1316.0-3338@sL^`=Wy@<ñÁ'°—À8I[	T=À;6jEî÷š?ã˜ÂÁÜö@Bv2aQ)@"ül—¿à*¶Fšæm¿åuµÃ_ªy¿å
H@5¥(¿æîÅ%ñAGNfsrq?ïüNàbÖº?1÷ÖhØÑ?/ãÑuÀEI?)œm`?+.*Ÿ+ó%?"òZ+fw?ï±;Ì+^ ?ˆu)ˆ·
?qˆªÄqW?'a}›¦­?uÙoDèÞ?yvÜO֒Ø?ïLö\úÛ?'¦Š—îª?€ô…:Iww?r8~×5ƒ]?‹Í㞣Â?|gŸ Q?ïÖMXg9?uÇ
ÑgüÀ?3$ޞŒ
ô?BÎy£S??s§ñ¼/n?u_ãôŽâ?ïþ8æ.%`?!ÞnáÞoÃ?!»²º¸Ä?\ì1)?©À©ôѽ?PZwUåØ?ïá€V/?;?häˆ&;ëI?ZàŸ×êÝ?Uªµúd÷?aYÁÊæ?aΔ¢_Î?ï¢ÄDVàÑ?tl¸þJ[‹?so?þp§i?e85—|ä?{.äKî?p–)¸Ž9?ïøÓ2íh#?Q<:¯†?»Ã?›Ù\Á?Iƒ€|æ
?PÕ¯BLÿAGN3FGL J1317.8+3429@UÀ4 -œñ@T-€/eHÀ:7m¾I|KÀ;ñò';×?ÊLNöeÕû@›ôgÆc@«Jàxü¿å(­Q÷x¿èYV¥ÿª¿á_«ÀHì¿ïÿ¸JÅÝ+AGNfsrq?ïêR=Sak?wÞ7¹ðÉ!?'!ié9(?2;ýñŠ‰ ?d;«ïàâ©?wq
têÕ?î>¦€ »{?²9¦™ß?ŽºvÊ;ìÎ?)ÅGޖ?¤fúJ‰f?±Üúíli?_ot?¥f+ø¿4'?‡ÞÆ'Ûk?tÃM²¼[‹?¨_ã°íæ?¥Ú~7Ô³?"*«?—øÅp"nÜ?—­vïkJ`??¡h‹}Ï?"b6‹?TM?vt©ß²º?ïž!7Õ{¿?µMÚð?/ÐÞƃEû?Aè¯ä–?‡ønžë©a?µNñË¡ä?ïWgõª? Ð¦''|?v)÷8ÈÖÃ?qªèK+k?ô¢? W…—Áîœ?îÑ{œHê?™oôÌɆl?ƒïlêÐø?qȗy$úK?›ØÕø"Cª?™&îÄRܚ?ï°ôF¹M?r6o9Ç?{PêYÍ?h´‹6!H©?hÞj	°AJ?fþò*&´"AGN3FGL J1318.7-1232@s"¿Ÿ‡ð$@HãÓ %¤ÕÀ9³ '²ÌÀ;¨—¤¹¿ï'Ž>;@™íÎ à@ǹà`þH¿äkB	K‹¿ä¼0LÎ嬿æÃq¦­Ì¿áÓÞTð®eAGNbcu?ïõ{2?NŒ˜Í*Öâ?@¨¡q00›?>´Êš<?Ikræûð?FÉë7á§?ï­óý­H?ˆ÷óJ¾T?ssLSñ¿?ƒŽ°Ú˜?uÿðh:V?{Õu?ïI'"?€c|×äÿY?-Þ~๞?qZøò4-a?Œm|˦³¾?w½ûÓ¿h?ï~‡AIû?ƒv±Œàe?M"S–»?M]¾ˆ;Ä?Ž…?}@?ƒæ2»Ê_?ïú ë®?X³YoÆ)?1`d]´Ÿ?-¼w¾YÔY?9r]½Þ6?XQu˜Ð?ïåH"d?hے92c›?WyÜñÑH?VMƒÂÊñÒ?^XTÄ?cî¦AïÎ?﯉‰ÅÕÑ?oq•äQp?r5#$Ö¤Á?iX(JuéÂ?vÕâZ¶?^åì>Pù?ïçê*^Uÿ?_%F–&on?%µû¬wû?½&ß$È?fºuö"ýô?^ÄÍ9°+&AGN3FGL J1319.3+1402@t¬–ÿÁß@RØû_ò®ßÀ:Նjè¬&À;ýŌf«0?ãPŒ~^ú@H§Ž¤É?ý؜žÜ¤†¿é•Øa€x‹¿Ùï38'—¿ÙDh(¢$q¿Õ¤ýä$Š×AGNbll?ïö¡'­"?HÊ(y¨?@#HÁ§5'?:†96''Ç?EVo¶ŽÍY?AÌ"‰…$?ïz¸Y–
?'°4£'8N?€FYÁS?†G"S˜´?M£ÆG
b?"KQ-­?ﲦ—??"ivyý?ˆybõ÷3?{8Á0?'Ìù«B²"?y²à
Š|?îtb5‡ÔÔ?¡Æ×üfÿ?—uW¨?ãðfCð?™þ7ñ…?sÄ.(îr?ïûÙ¼è?4Íë;Ç»ý?/+»Ó®?&Ó˜D{?8cUûÛ^}?-ŽÅúg×?ïØÊO!®Ú?pè}™¿v?b·ÄçÍòx?eês׋=F?d}ì7Û3?d·¸Ô(Q?ïÁJ|iÍ?tðŸýÆEÈ?{ÏQèŸ?l‹u{á?'(!òdq?hOž6?`F^+?"¤©S\/?†2ð°®h?aÕÌ¿?qÑýQÚ?knœ—…*<AGN3FGL J1319.6+7759@^CE€<ÑB@Cƒq_¾¬yÀ:2ÂfA}yÀ;äÚÔÍLO¿‰9	`üÅ
@—½Clç4?ü'_øc)¿äé»Qп×w3£E"à¿å²R^OI?²×œù9VAGNbcu?ï÷í@{?D†_(cç?5©»Ä$Y?2y_WæΞ?Evä¨vÒv?@QügLÚ?ï¬Ñzî?"+\3¹i8?qlC
[‰?qæQ3¼U?x}֗ÁE7?QÄ1_€é?ï?œº$Bn?'®0lëÎã?†$[œ6k?xL~Ìí?‰ôuá˜0Å?tÆe•10I?ï¤Â_5š—?ƒZÍñ?SÏ]e«Ñ?\¸ÐôS>?"U|'Ô†Þ?€Ž
ÂôÃ?ïýî&cÂ?,à9Qâv.?":[UFE?vì†IՊ?-v'Y1Wº?$8˜ë·ðÃ?ïàŞt?g€ŒâŽñ?[žéà?Të­Sw"?bù¡žK1?amš½§,?ï™ÚIb®?s"ÖÔ2~?yÂSõ:8?mžfiÐL?yP‡tƒ€˜?c÷l¬?ïó>¿6ì?Psà՞ԫ?2	è2ùð+?/X'Zß?U‰LŸŠ?N¯ xàAGN3FGL J1321.0+2215@vj¿ß~€9@TlŸëWÒÀ8ÆÄŸäÀ;zŠPPzl?Óô½¨RÖ"@YÌ­ÃJ@_ÄŠŠ¿ã–¤'çã¿æݳ*u…¤¿âÐ1ú+³@¿êïgMä[×AGNfsrq?ïñ¶ÆÑ
I?l¤eX{Œ?Cvåû@LŸ?OÃ܂d?RÖþ𱑇?g.û·?ï­ ó¼6?­ùÀîï¢À?tø%‡£H×?{AAg4X?˜ìB{()?­ÏHÞã?îL×vÉàß?ŸAp–H´Ø?‹9TÜç|E?€Õp—½*~?¤d3^»Çù?žNþ­ÔëÓ?ïkÕ¬wö9?‹‡7Ym
™?rç¾gœ­Þ?nß^RyR/?‹–µž
ðÏ?‰lÃ?çP?ïùŒ|z¥?Uïü%·:?@r-¼±Ê@?K!¦Â:™?6ÿAÞV•î?G>GZŸ?בּ/H©"?ï/Ž":?ã·ƒ?^*0
¢Ûä?€`°œ¥õ–?Ž¶îôQçw?îð÷yý$·?—­—úÉd?€"×WA?v¶e}ÃZI?™–¥,ü‹¢?—ut=—ú®?ïå4GZ\˜?a©uR:&?U	¿'cáÅ?G%Ø´¢ž2?`FØß±'>?`
ý]%,…AGN3FGL J1321.7+8312@^vÖÿ´@@íÛ L¦¢À9ˆœ×;»˜À;å#ôÑΔ¿úŸ-èE¤$@¿:òð"@"ÿï¿çÿÕJF
¿å[ËÙæC¿ä-"XÐâ¿ìຍZ)AGNfsrq?ïöŠ8'¹­?W‹^Q™?Kz'¥?T÷üc¹É?5‰I¯œ#5?1Ò¤§w3í?﵋¢µ÷ô?€"Þôj")?m/U¨ˆÖ?mÝ€¿m?v¢ƒð\k]?yfÍ!	Ì?îþ·û{Ù7?¾Lw?'-Wg?ˆPìh?‹SòÉË5?{$k´IïE?ïã'Á~Ô¶?oÞ^[\H?+Û×i*?>"nâÜî?k€çøsƒ?n1<u•›?ïöìÈ©?`¶99;ó½?Mþ%x¥?`ƒ]¬©LÝ?):å©!\³?$ÊxØØx?ïåG,U?eŠcû5îŠ?X(DØM9¿?U¿ ÅP	?]Ib@KÏ?\XPêÏO]?ïSËÕ+?ƒ`°‰iÝ?ŒöUñ??qb¡hy?~m­ß¢?i:Û[?ïüOžp:r?H+mw6>ðI_Q*?	Rü©?<~uþ d?Gïpþu—AGN3FGL J1322.3+0839@t_._ú;›@Qˆ¹`~TÀ9êk#d‰À;ȓ6©	y¿í0ÇA-Øç@5KÈÊà@D_ÖT`¿åªü°•3®¿ææ*cMO¿Ì-Ìnâ¿ïù_'aÁçAGNbcu?ïìb',E?cºB£3?KLƒ¡¿_?MØJ xÑ~?Y"›µ(ƒ?_ä¥dà¡?ï™ØZì×ü?‡"!\1‰Y?w~а© 
?y.©Ó!÷^?{•êÈÙ¡?²ç}cL?î?ª·›"£?š"pwŸ9e?¡Y:ð$?"2ˆø4¼?•X3#³?ˆýñÜŒ]?ï åщ'º?S/­b¾W?^Õ!ûíh?fðӂjžD?"0ø»Ò?q%ô¾¨Ò?ï÷ú$@H'?KHÕDŠ0??¯®5Š^ê?<0ៈ.?@?˜ÔxÓ?Að~Z¾7G?ïÛEÜIÜ?nÁ¹›ß{?a£Èôßf1?^9¿¥+"
?c[A0U??eÎÄJԃà?ï3ê=K?‰tPs…¿º?""$©=â ?'ë[ì¯}?…®¼(€Jë?|·/ÎB!q?ïî²|´Ã?Z"˜ßÂR?8z%ÿîx?@•¯"(@Ç?\}E÷Ã1ú?XO÷°ŽpAGN3FGL J1322.6-1619@s›§ÿyÈ@FòÖàL'À:…zþ£ßÀ;´°t§qÉ¿öÁÊóƒÅÈ@
my=¿Î@Ùö X:)¿ãØ_'.¿å‹öº±í¿ä2Äߝ׿äuø»Ï5AGNbcu?ïœt59¦H?ˆ¾"ÉÒѱ?a[ñd$ ?gäsÙô?"‹ö`‰ô?†lœvÈÓ?ï£áؼ^?†_‰Â$ìã?s¹r–
D?qϓd—øc?zU¡×¾H?o€Û '?í¾eǍ¦?škºÕuà?•"´ŽQ?ÍÐ_(Üz?©—°•œzn?•	è…;Èì?ï"iòëx?ÀÆæ 3f?W#U	à¿?T•éü%‡?š@'Iü¾Ñ?õªpê>?ïìP˟{0?oC÷µ³s?A"ÌÅú9Í?AèMÌð"j?^"'¹Ö?m,Õ\X?ïá>¥=wì?iÖQÜÏÊ?]Yå¶r?[óۙBð?`hÙ¤?`uØ֏©	?ï7
9·(?•¨è{ÝÒ?êþ]2öû?iò‡eË?'?'šªn?|Gù®úU?ïÖ w•t?gœ»÷)?0pÝ­Ñ?*€9aMµY?sõèº=!ú?g:¦Ö)SAGN3FGL J1322.8-0938@s»î²Ñ@J9JÞ™À9ò#žjºÀ;—ÿ'E7?ßÕs順â@½×Zob9@	Ÿ#•¿ç˨÷ý¿åäÁ ØMñ¿ìböuÎÊd¿æ6É5œ!½AGNfsrq?ïüÜ
Ç$?0ü˜èHi?/ŸŸ0åp	?),a;êöÞ?"Ÿ²ÊÜtm?!#™ÌÑ°@?ï°V ÀaQ?'TY¸Fò?q&''%Œ?q [A|œ"?v¹É-9­Î?|t#?ي?ï·6Ò=ê?‹{?²	·k?…ê]<­@§?yD%GÜéH?"ꅩÔy?‡#†_-¡Ÿ?ï‰+…>î¨?†€ãÑ}Ã?ny,£¥v?gŠÜæ>?†יʤ?†ax›J?ïþXMÒyh?!Þ"{Á? ýžVtiè?'T
r¢?ûQ&í4?=¬‹JÌ?ïãjw[ðÛ?i†ù&oœð?X¸Ê…‹O?Sˆî 聁?`9#i¾îé?dDZmI݁?ï|¶ÿ}p'?'|·fÙ/á?y€€:i?m‰–CZ<?"ÿü	j?€)¨ïÇ©?ïêWq^›?dk›G¯B?LÝHWX®?>çÀNÕG:?]­qó¤[?bið•"AGN3FGL J1322.9+0435@t,@FA-@PìŸÐë?À:_nÔÉñPÀ;³gþìډ?é
Ƨ™·w@
¡×ŒÄI?ûÕP~ó{¿ïÿɯ"‹E?ïúK"	¸¿Âá‡é\¿7¿áfŸ*ÀAGNbll?ïõšoò(?N®òã'T%?9²(>ï"?6r‡µfÉ[?L½,䅃¯?Ggº"@3ÿ?íŸh Xm³?´½Òf"'?©Lýêág?°î3WxëW?™zÉÿû¾Ì?žlXÛ?ï‰ÞTxl?'À~8SÔJ?"ÐZd¿6%?q"ó&v4?'¦–ü2u?}H'Vq(õ?ë
<ðÝ^|?¶züœœy
?ÀU•ˆ½Ô6?µª¸9'©Ù?œµ£ŒøÒ?˜þ¤˜ø ??ïú7…—?=ÃêfYJj?-<c½hëê?%ÇêKß J??¥¢±$ƒÆ?7Ù0C´Ó?ï~¦±…·?ˆ»"|±>l?ƒM•êJ|Ÿ?€ðèo…9?z{H×Ÿ?w=(LHÜ©?ï‡Ð‡¨'•?p"ú´Fy?y	Vr?õ?e<Kª_Nï?‡Xa[ˆ¿?e®?"î?íê»hTî?Ÿ¶‹&k"?­¤]ɳ—?7I~ŠZÉ?}]Ž"˜?zl+1Z¹AGN3FGL J1323.0+2942@Kš¿¨!@T¦$`1˜ÿÀ9Τ…À;"Å@'H¿ßÄßv%T@.ëí¤^@)KßÒc¿á~ÚxSp7¿àQs.ZË¿å)zûÒQz¿Ù0àí¥AGNbcu?ï)ë9°Œ?œS4ñ©o?|ÎM,¾²?yÞO¸_Ò?"a«Ñ?™Îf9vÂu?î¹ øÕa?´aSÆRi—?ƒü¹?ÏhP?•%gÖZh?žÝ¢ÝåùÄ?²úÐ覢5?ìÉGþv? e?¤úƒ'?¢ñ;ìÀ2?"Û®õè?°=>™=µ5?™RWã,:?íÇ6ƒ?¢5ô('bœ?AOãY?'us‰4}¨?«oUÖí$? 
V9*j£?ï‰ö,'âX?®ž™bÛû?hž̑=S?qêl줛?‡Zó²
«?®<[¹¯Ñ¤?ï \Q@?šAXB"؝?kAPý~‡?}ÄÉ
±òô?ºTà‰?˜GDA‹V.?î–_÷ˆ?"·Q<=?"Mj~êdå?†}Ð馝?™æµ$fF?Œœ1¬þÙÃ?ï•sò7Œ×?{zU7"4é?b9Ì'¬?U&tXë?†e%d7?zt…Âw3AGN3FGL J1323.9+1405@tì¿ðEx@RºÅ_ñ_À:1Sϊí.À;Ñ#2ý?ß;¢9¦@¡Û1"x@›·1Ô?ïÿ"77y¿¿Ý^?ðt¶z¿ãA?ØTŒÂ¿Üã?AGNbll?ïò™­œp?gà.ºç?5®¸-ͺ
?1>ûkï?U`ö²ÐL?fÀü›Ü¾×?ïaM÷?œS|Ô¼Û=?ƒ1T/l\?"~¸ÀñåE?"{.:5ª?²Ãnü£Y?ïÉVB#]?‰Ÿä_±-™?Š¥ŽÇ
8?'uÅù¤¿8?è¤úŠp?€.š\ŒÕ?íÅià­?«Ýö=O	?¥l>Ëûh,? ÖíÊä¹T?©×j£v?¥5¨¹Š4S?ïú/—§?bF=÷¾ZG?"!kI[™?å'?""?AzéIìó]?b0êyH$ä?ïÍ4›	©?€§ÏQéÚ?kl£i–?w÷¡‰&)?gt(%úï­?o¬7͔ýa?ïEƒ<#á?'¾¢É‹RC?"BӇcN?†–-ç4{4?Š]†míÄ>?ˆPÉ;à»H?ïa%ç<²?…ÿ§ïÌ?†¸#×Òb¯?wzf'ùôÑ?€þbZþ5?~ƒª="†"AGN3FGL J1324.0-4330e@sR°€0<@2ú!€ƒHÀ7¯¦Ç…òÀ:4>ª_º{?Ó°ÙpcI@O92¦›`@94¿zSٿ僢k80¿ésr࿕¿ç4ú|»¿çRÌÒ<^'AGNRDG?ç¢Êã=§€?Ê֚Ù/ø?ƒ$äœ:so?Œ™éHy?Ð!CBKC?ʞå9fdI?ï{>õ´!°?œ§ËKêÐ?vm¼éLV½?wJýzÏ´ö?…ùdQh—?˜4É`[µ?â«åGܧO?¶Ì£†RK?¾"è¹éé?«£S|ŠÝB?Ó;mX6è?´:|¨¨?å"µ¯#ï?·ýÇìhH"?†‹îÓ`N?€ÍìY+õ?Õ43¹@?·¾†¼[á3?ë2Ï12¨?Äþ§Òä¶E?'Ût0…?^ú«:'…?Ââšc÷?ě³M'ƒ°?ïÅWŽ¾Â?……Îe?fô4•ìåi?gKæÏŸ?qÚXö™(u?€ê¿zIŠG?⧢V#‰?¶òAMî™}?¿X
Oš?¬ƒWÃg?ÒÚ¸‹Ù?³às'÷?éùã¥ù›¯?«iú=|b?}YB¢KÒ?l«X-š?Ç-§Q¬ß¶?ªûL¤ãrAGN3FGL J1325.4-4301@sXA?ÐÐh@3gßÿ¯x(À7oB¸âÀ:ç|8_ÂÞ?ê1M*Þ®@U8âtª@Ÿ¹<:ï¿è:ªmHпèãÊÀŒ¿åÀæøД`¿âwÄËT/`AGNRDG?î錕>?¢Voèå?—2T+Ÿm?Ÿ ô§"I¢?‡rv'¾K?Šu,°Ó–?釯SU_?Î6‹("ð?À^?nˆ|n?ÄméõI5?³^œŽ.?À~ËYê?èÿã×D?«î¸äE`ô?¸É¦Î´¤$?¥Î줽ì?¿9lªš•:?¥ô7ÉÀø?Ú
.1̛?¿Õ5bu&?Ê|ؘ²ê?¼8Ü?†}³?Øä"bÙð?ÀÇïi(—?áDÂÁ?‡a‡%Cû?=:}gOi?ƒŠïŸm²?qÿÔã¦ëØ?r?ÊJ-w?í"cª3?Â?VTþè†?«Ú_ëú™Í?¶Åû3ëÔu?¢MYÙrõ?³‹¨Z(?ê)©€±/&?¬f4¢«{?¶^ÄØó<?£Œ+3>Ù ?¸Sï!ë ?¤nĺÌȅ?æa—Áõz¸?²°á,s?»}Iñxu?£§Œ+´ô?ȺûÿjXä?±0¤Z	XAGN3FGL J1326.1+2931@J8ïÝëÙ@TڿԖÆÀ:²/ÍM%MÀ;ѝx]¿ô
%\ÛÎ@…"'|Ç@Ž@?`=-¿Ú˜D¦3l$¿é¿F™cá¿ç‹ø&Ì{?ÊWÍ.Ïÿ»AGNbll?ïñLn¡&	?` ¸Se`?5Ϥ°z?8›!,k0?Wó:P›"?^ÿBÂ|¤²?ïŒÃh±*–?›,tY'V?f¾÷Œgü™?o'-Ô»?‡gÿa­A?š¥2M0ê–?î£ î?•2­ñ">/?ˆ[Am~JÃ?}¦'2B¡~?Ÿo{I2µ?"["DµÌ?ïߔòã.Z?p‹$ö¬\¦? ¼Bm?
xž†T'×?paQk¼î?paÔ?ïò-—<òû?"D9>/Ӓ?0Ía–è¨?:<ä2èÆË?WqyNÔY?"&UE'	®?ïÐXOäJ?Œƒ7M6N?T)íƒãd=?UŠè)^C?rÉ]0!¥Ö?‹/Pa<<?ïJA˜.h&?¾¸vL?{!AL»l?pxEü®zÉ?ßÓ¬Ò?ŒO4pú?ïüÉ&¥^?5o7áßùÞ>Ø^Ÿd±!ÿ>âi¸2˜ƒ?9UN?˜ç+?5Cƒ×%/AGN3FGL J1326.6-5256@sDÊ€à@#!Kãö	À8?ŽîDì™À;}\L11?æ%í‰t¢-@•‹$‹Ðƒ@ùÀ›f"¿åȨͿäʳÎ+пä±m7ˆNæ¿è|¬uAGNbll?ïñåÃ|?Rý
2ƒò?Hl=ãCx	?E›´ÁÄ¿?OýÃ
²Ø#?I}¾ÿ¨÷?ï
¶yÀm?£°Ùb(á?t;öOKól?u>è0Ë?™:3IÜׂ?¢ŸÎTöÍ2?îzÜ©tê?""Bñ»?'­€¿°Â?ƒBTÈ^?Ÿƒ­kø?L
?€?ïµÀϜ£?}'cŠ"Š?D2û(×L?Pd.Ö¿®C?O¨ùw¿n?|؛7€9?ïûpY|a?<{3b~xè?4‰7™¢šP?1›èNaÈÏ?/è%-š¢?-ôAe<Ô?ïºäG?€7Î:B–‡?_caôC¸¬?Xˆv0³Ñÿ?zµ
š?}f·VZ`?ïde¡*ô?D|ه׹?+¼Î}S?qäñ£õ&Ù?‡P¹`FWK?yMPlc/?ïîwf‹F½?]­
ž´ð'?3RÂ];÷I?0ÓS0clr?^<'VÏÍ
?\ʊäOAGN3FGL J1326.7-4727@sQ§€w‰¤@-÷`¿]xÀ9]5õ…R»À;ZxOœöE?ýèªMñÐ@È?ânÂ?âC`èo?ïþ¤žv¿Ðû÷\ÃOv¿å­Ðrû¿îÂh?"zNOTHERglc?§òptnˆ?¯'fÍô¨?îg2zëG{?°sε®mÔ?i¦ƒ]Õ4±?rv"b\±?¸´q¾¬?¿Û5äFÇ?é"ú²?ÅÇ֝ù?¾;Š@qpl?¿n^h§DŽ?´'…,‹?¯/œÍA?èó£ Ù~â?° ^;?²ù½ûá}Ø?¡éŸkj²?Ç"È›Ý
?»f²!áãF?æ'i܉ûŽ?²Y2?½=‡Šxis?¶ÓäwIŸ?¡»iM š?®R7éXý?îØâÌ,W¼?¯UÔÅUn?f}57RÓ?w±Ó ù?ʕÎB¤y?ŀMuÝ/y?å¼£JBw?Ç×¥:Y±?¼ïJÝì&Q?»£ÐD|?Þ2BÆà?­_°¸°e?藩"É'ý?°Á~v°?´NØ{Ù?¢l½3µa?Óڙ}ƒÓ#?·8:a®Ne?ãٛiþKu?º—t?0Ü0?±È¾¼'Ê?©ô'þŠ{PSR3FGL J1326.8+2211@
o}ÿ_F7@T#kà"êçÀ8¤ðÂuZöÀ;f's"L?õ-wTuM4@"Ëõak€@svënοâî›
²á¿æ¡99mÆ¿è›–ýïܿ璂/‰tLAGNfsrq?ïïyäÈu?[7>ÂrÕ¯?WëëO‰ ?WQŸèç­?BCõÈK7??}z'¸ÜU?îÿUš*'
?¨›CHò;?'´€
¶l?ˆ'.ÀÖg?—òi‡?§=";ä?îíb~$Q?'c½I	$?'ÔxƒB–Þ?ˆ¦9•@ý?D§Ñu?"Q±äl8Q?í­§N/?¤'Ë{,á?¤­•Øwƒx?#'_B? 'O¸€š?œ¼ÁË«©?ïù_>¡GÛ?Cf¹V,ú?DBúí'Ð?@†ÒÈכe?),[#:Ô?$n.^5¦?ïšæ[û9®?"ÓȈ}9'?m?sœ?{ـÂ5ƒ?ã8ää£?'hsùûBÒ?ïU+ ü5+?…vžàô!?‰>Xå¦6?bÜð»§Q?£ùgµð?tZ(ŒÞlª?ïNÜÎfn¹?…Ûié?ّ?·	RJ`Ý?|Ð5­•ô?y#†EÀ…Â?y7"}äAGN3FGL J1327.9+2524@7·_}>@Th—×5ÜÀ:üײÙ܀À;úé¦Ù¿®É÷G")ï@Æç¨pL?úڒ€Ê÷¿ïÌ»N9Ö?å¹Q
ô¿êlMäF?áªÅK#>ôAGNbll?ïŸ='N‡?'ä'" ?vUôÛ_
ä?'Ε?zB‰«z™?Š@S")?ïŽ~ø¥åû?—Ó9.'%?n›Îdhë•?vX99 ø@?"¹NF³8i?–¶¼îrè?í±‡–¯%ê? ï´ÎìFA?•çÆřA?ŠH°š}ti?©ó£1e+=?Ÿ«
GVÏÇ?ﷅ»i?ˆ(	`0TL?p¹dâ$D?"-ÁºŽ?s"` Ÿ_f?{†+^Ŷ˜?ï³¼>~?£ƒÝl?c5Å*âA×?p—9cj/ä?|†þkC ?£]ÒPìÃ?ïÍO€4²~?'_°¿¥òÃ?Y@>Ì&T?_¼_žÎp<?s0ñW?Æ£b&à?î¶Õ!?•Æ7çŠÙ±?‹Ìƒ\ހ¾?'úSÚNëÍ?›?&¤.?"[ã~àÊ?ïøQ,dÚB?S'Zé}®?6¨¢·›?Al:K«§?CYù3—?LNû	NôâAGN3FGL J1328.5-4728@sVž²gÇ@-Ø->ýkÑÀ9=E†SÀ;2îiՇ¿ò³CÛ[@T¸ëC…f?û0ßÞøH|¿ïëâ§)¥?씪¯Ê8¿Ûù)ßCê2¿"uv'EóˆAGNbcu?ï扙=ˊ?(©Í‰Ú?FéÇQw­)?@›¾‹YpÈ?c»ôª7Ô´?€ý¯¢¥?ïŠïâróµ?'¸<ɔF?oL¾¥¼År?m¶÷¬jq?…p×½óid?
‹ýáB?î…îCe'?'ü!¥?'ú/w
$P?"$`ûW]?H
‡hnÈ?Œ‰aËɂð?ïi[w¹¹¹?'¸Q?¸§§?B7:'š?IªKy?'CàEŽ°?'¨Ù*™?ïëŸÎgÀ?'ròYÜç¸?8¼vIõÅ÷?0'%ªìç?aH£?µ6?'tvøÄrA?ïÙàZ'Ã?s$µ¡ÙJ?WPcÈaæ?RTª
]#?jwt¼ê-?q	QÄ$?ïO¤5²r?"¯Hhµ²:?"¢ò!´Êf?{«pUƒbF?‡t`€¦â?|Z´ò?ïÕMôÌès?h'ý'¶ÚF?,œ
C?
;6ÜáÊ?tüU¦z¨"?hnB¯¦A
AGN3FGL J1328.9-5607@sBÓ@N¤©@nÔ?²ÈjÀ7`>"E]À:ÅÁ:c©?ü©}å‰N@­ègÝßÅ@sÃ²ñ¿áäŒö·Ç¿å¦ìXáÌ¿æòhElN¿ç?¨ñóš8AGNbcu?ï–l-z·?–×Ó¥©ÔB?ZÁ]"?\őɆfJ?‡QZTy?–›ÎeØ?îâà?f·?¤ÑF\šZ–?wJn‹{a?"f]ë>,?ÑaîÜQ?£%—‹™É?í²š2,X? ]ƒµHû?ž·°\c4?"|è
9X?¥z͆Éç?—î>R+?ôá$.?'ž¾}›åŽ?QBàmE*?^B9s±®?‰¼:i™‡â?'dÄwT$Ž?ëÅÑ©^_?ÑP§ÉnZ?v½Ñ†–Ä¿?™ã¾±r?À2ÊÏéÚ?ÐÃnMÕ9È?ï˜ifS¤ ?™ØU.?cƒ\R¨¤½?h}‡î‹?…ÏUd̸?–~^½$Ž?îÑüÊ"µ?•×,
jª?'< *"¢?‹#Áð·?"ƒÝ3'Ö?ŽJûgD%×?ïæ
öÒt?h²ßEâA?K›²(³'"?PÄÃM!ì?bûrÅ?F?ehm¤qAGN3FGL J1330.0-3818@ss?À	oë@7ð#¶eÀ9´8ù€ŠÀ;u±ƒ›*"?äwɘÃc@
Xâe,@>Úà5à7¿éÇúÇÔ7¿é4ÀÜ©Ž¯¿ïÿ	(®Ü¿æäy<_Š]AGNfsrq?ïN4a£å?ªb¾·ÇhE?‹rª:¨QÖ?"pH¸6°?=a½8Ë?¦å:lb~Ð?ì¾ü£æ?Æ*zÊBü?³š"
¹ls?½~¬K€?§þ÷º?¸¯hêz4?ë^#2£Û?¨Ob1Ü?¨))Ö#t?—¦Va"¿$?¹ÑÔ>HJ?£¹ZOõµ?Ûq€;ƒ?Â:]fÒ?×h@€Îœ†?ǜ/œ¶ë ?ÊL~çDOï?¹*ÄC6A£?ï֌SÉM?;\¸Ü¡?fÆ!2®j?uÝ­: ec?b­ájđ?mŠ«c÷Ci?î{Cí+?¶±áS¶n8?ŸÏà¥;?±v‰J‰>—?'²fÛ[z?¤kP|Œpü?î1M™!4ê?—±*xÝ3
?"ÐÇòìs?…
uPiC?¢ƒ«	"?"fø{Š?èë'Öג¤?­k-µð½B?Á}¬!ËE¨?ªdÜmf¦K?µ¨d­'?œ"u{ÏñAGN3FGL J1330.0+4437@YeÊâ°@Q·: þ¡À:V'šx¼ªÀ<¯ÑêC?Þݳ¹DHž@rѹp¤ƒ@4¬¥Q´¿áþØöPÔ¯¿Ð×ͫοá‡À[ØÌ¿ã@	ʦyHAGNbll?ï󺐽±?U 8mþ_ë?:þ
èÊ?7Ö´Vª?S!†¿
Ó?QæTÃÕâ?ï*M8†£?š¼aANÚ?‹ ˆÀì4j?'PåÆ?ŠL)EÀöÍ?Ž%Á#¯O?ï+`qëæÕ?†sô(aÙ?…2€vVQ?x	$'»Æî?õcc?=x#"ÁÕ?íÛ©% 	?±.¬Ré8?¦œ±ôPÁ±?—5>š'[?—QwkòA{?DÿaÀ&†?ïûŸƒ»?6ÖÐ'?"~zÇÐ?¥¾¿[ÖÔ?9È)°céä?2AõÂ3ü?ïÁŸËÈüð?y¶—¸5>?nŸÁžx¯?p§ò¾A?oÀsIbw?pñ£o&?ï™Ð›/é?p›¬#"?uÞ$Ö&§Z?a@—çì"?}9¬Ñh?iÔ-tói?ïnzT~Œ?FŽ£?‹ï´÷_?t	hȺ=?pãm¬
Ÿh?o­D'šAGN3FGL J1330.1-7002@s#ý@gÏÀ²mÀ!î'À8ñ'lÀ:óyˆ'!?÷vÏtòÆ1@ã[vsN×@:~äa"ï¿ÝFž<
å¿å$oÅy‹ ¿æÎb("Ú¿å íÅYª°AGNbcu?ïÂx#cmŸ?w"à¨`'?<z€à—}€?7Y-h;i°?|üFYx
Ð?v'­³›½$?îË©*u
b?®\j>ý÷?zþ€Pñ€?…¶­V6"?ŸËU6U?ªJÍvÉh?îêy
»ˆ?érj˜´ž?"ÞË,,¼s?Š/Õtó?¥aòÜ}…A?–ÄŒc/'?ïÓÄ\T®r?xß áEÛz?*ÂüâÂb?72±hȂ'?uGÁEì.£?xÙÝXï†?ïêG^¹Há?b©ÓØ"ß?:4lª":Ü?7é£É#š?brz$™?`Ë© ÷!¯?ïŽÑ—˜k?'‹F˜Z®?g'ðòÞ9Ë?p'ÒNš®?†jãèaµ?ˆ9Cd"?ï›ûɏ?KøzEX‰?‰Ÿ¶9 P?|¹"ÄÌWò?'œô(A£Ë?…åƒ{?Ôf?ïöì72
?Rñíè®.A?%ú88ƒ?)
ôŠ÷4?O
P]–_?Q×\mH=ÁAGN3FGL J1330.5+3023@L­ŸàÛx@T5iÿãzŽÀ:7²€fÃÀ;Þ¬k-v¿Ü E`Ãuq@
P¨ø².@ÌÀÀz&¿é©Æ}Rf)¿åãÀ.XÙ¿â)î`›KK¿ïÿê›ê¬²OTHERcss?ï±òMå¼?…ÒÎ-Dè°?bEß*Æ?iÎE@¦Œ:?}ãé"ëÑh?'ådc õ?îðýÂý¯Ý?¤dÙçpÌ?—ÅpÕ-®	? ††«²?"5­…b–ª?e™«Åè˜?ëö|ž¬O?¤üKOë—í?³t0°¿?Ÿâ"!À͙?©¯3ÿsِ?˜j25ß?í0²ÉÛ°?¬,܈Õǵ?­ûƶd)?©•ê}²?óƒ5x3£?"mý'£é?ï³|ýŠ7…?ˆ4`³2¬?a\䲶Á?fO)ZÚ¨–?}"sÊ1?…'õõìÔö?ï´6G(¢O?RéDôD?y£e›HÜ?{:y'®éñ?h'îÒD&¿?p¦œVZ?íLƒ–¢ï.? KòLÝ*?©Š¤™ˆï×?—†kn¬éª?¡­!ûl6N?"W2rÂ5?ï{EÜIÜ?~ë!-Ÿ
?…©eÎí·Ÿ?x¼Ÿæ?w
FkNv"?pæƒëÿ
kAGN3FGL J1330.6+7002@]"'þKÊÚ@G\ @hÀ:Ì°G[À;êpçɨ¿ø‡ÁªÚµ@íJsk²?ý~©E¿êö5ó›²g¿Ý3"N*ý§¿Õ	'oß¿Öˤ®YMAGNbll?ïþiÔ°q?HO‡Bp?ê6'Š9J?à0ο¯Ö?ôëêúOÌ?&Ô®	?ï½ÓµÃX?|¾bwÐ!?lˆþÙɼJ?mfzòˆGá?rÑ¥ùËÜ?u[›-«O?ïxٝ7*[?uFçŒ>à?y¸óz®@s?fGî&(?"íüÅbö?m†"È–Q§?ïÙ!þ=ÄB?i`«·½í?kÀŠ?çŒOÐć?s!QÏ¡R?i7(l{Ã?ïþº,Áe?.êÇ$«?PúýÍrˆ?¯Ò»!å?n›5Ò.ô?@š
Æ?±?ï妭Õ«?c!ȹ'?X7®
352?T¯ß½P"(?\z÷yh¬?Y_D3å£q?ï®à2…8d?kt…_&?qŒüü/j?cë|¡yµ?wé¯}¦à?]ä~‹ŠŸ?ïù¡úï¨x?@p,‹>õ"ÌáUó>ïÆPÌ}0?HËm$é<ô??ؾ«¼AGN3FGL J1330.9+5201@[>Ùb…U@Pî`/ë€À:{ÛÑLŽNÀ;ôy±œÅž?×í3¸Fán@öÅ&@ýp N¿êœ.Á¬¿ã†6TÈ%À¿ë{䖱Í?Úö'bñ;íAGNbcu?ïíÂï1a?b"ž1K'?^ÓˆžŸ;?aÚU*uÝ?6œu hð?1ªò;¶â?ï¼B\W*?'ëÞ*:h?mfU?'¬6?tóϊŠ9­?s+§uQB?x'ë\?î›At"|y?"ú´Uvmß?—Ââ'zÔA?'-a—\™?"ÔîÚ=Θ?!Ïbp9?雷à3~?‡±myb‹?`óay~.w?wƒ]!ž?'`â%tÓ?ƒ Gpp?ï÷¥]¦'?Q˵^:Ú²?IÞDۏX?N'As]™?0 A¨
Ê?.JÈ×иÔ?ïåbb˜?fá;¶Ó~?Ylb_‹ÍÉ?[V_
d ~?\Zš²s²6?Y—³Gåü¯?ïVÒåj¨j?ƒõòZÜâ?ˆF	d?ì4T¿?'IždEV?koKƒ?ïöÿáCŸ?^öõkW·?7u†!â]?PYܲÎiõ?L5=ÿzu?RÕ®­-ôPAGN3FGL J1331.1-1328@sØMŸS @H!ˆô'À9ÂMFðPÀ;GÔX²H½?ì,û¶š0@›3\"ë'@ý‰€qÕZ¿Ñ«óI¿áÙRûGá¿ç%RuÿDz¿îÒÁǜG…AGNbcu?î•YCNa?¥nž ðn?¦6ÎèÊô?¥*Ûpµ'?Lç:ü`É?F\C+uÇ?ÄÅÙ?¤îŽbìY?™š~_Æ(?•žÓ¦!?"0IINã?ž:ôc7ßu?éûFïõé?®0?¾I?Â@¦£Ã>.?©i¬Çڛ?§Höt(*r?–
kH5ig?çڙ€3ÿ?³(yŽêǒ?Â5ZàvLã?¯Ê;¥'?¼À~={>B?§NW:ŸDF?ïùæòy?¢Mt†q?›dÔ:áD¬?¢B"ó}Á?G}ÝJ¦Eê?AÕð
·7"?ï{W)]-?Ž"ØÙ0Ä?ƒRFA–?†brïibx?{¯æ"¡p©?RúEýJy?ëÍüššËs?¥ù/DOàõ?ºªT2mw?¢ì-¦Š½?›˜;b¼À?Ž¡æ°}Õ§?ì³4ätoz?™ñþh{Û?±>Сϐ?"»›Yß°¯?¢P"á´G?‡ZçR>AGN3FGL J1331.5+1711@uÀLSâÖ@S΀+3ŠÀ9œÔY‰RÀ;ÁÂv1µ…?ç¯hZSÖ@ڍ°e@žÿµ¿è`ñEcG´¿ê<¢óŠ|¿ØY‡±J÷¿ë¶?0†IuAGNbll?ïÝW¿.©Œ?pÙâ2g?jÒ ?êr?k¬öNk"ï?OV',S?Rè#ƒ}?ì	FX\–?¼Û­‡¯ƒ³?³mµî)Œî?³ÊÕk~?¨.™˜p?²Ñ ¨ï?í÷°O,|Ï?šÎúEù*ñ?›2ÿ2dQ?‹~J1Í?¢ë¬
Ÿà?"¬ÅþùÛÿ?êt|'²O?µ`Npy°]?¼Îʶ?²·"'ÛÛ?¯3ód š?¤M×2;?ïíý`µÄÀ?^"úDëq?[,¾¬	ù?Y« "1õ›?A±ƒëÒN?A;Ür?îÆ*jH‹?¢/öEt±á?˜+ø½|³ì?™ÿ0"u×î?ŽsöuQa?àd"L,À?ï"o!å?ŠQ—kNÕ?Œ+E4.ß%?|j'¬à?ŽïÞùå¹?ƒ§i"DÙ½?íëÇ4.Ð?˜Ÿ2ýÜ£Õ?«D´ø¶.?"cëþ9ƒ?ˆ± +ÁZ?'.êoì=AGN3FGL J1331.8+4718@ZDàÚ Ë@QŒÕ£5À9ê¶NÜ&À;úp¨È&?ã¸OO§×@>Âqªa@:ßßùû.¿â"Cׁm¿él®Ž6‰¿çu*ºúÎy¿èëáÁaÅÔAGNfsrq?ïöÁT•ûÍ?LVºð'œ…?CºLÎý,H?Cè+&}"P?A@aMŸùÔ?;Œ"_Æê:?ï5%é@j?—MöX"Ã?Š¿dex?ªºXtîç?ˆlð•À ?Š)¡ðóK?ï2k€g?}Žªl"J?'›àÂ-?qO]²w?mE\?uƒÑR
îT?í·ÄÃÐ
*? '̤;'?¦¤Õ må?•­½ßÙv?›¾K×NBõ?–zý}?ïû:ÁÐx?>,î1Ž?4—ûÔǔ?53VÿYÿ?1'ô¿Y6?,¼å:
'?ïÃ?°Í›\?v_öò|=?nõG2¶?mAmUnI?mËIÙT§ó?h¬Âjš÷?ï§JǤnà?ipKL›˜Y?so½G½È?aöì!?xêßã*|?]¶]è"Ñ?ï…!rÉÿœ?y/¨a ?†¸Õ§škÚ?ovpý«Ô?oû6d¼}T?lU‹ZØAGN3FGL J1332.0-0508@tـo&)@L!µ'm,À7rá`؇ìÀ:ìZ
7'g@b¶<g[@%8ZåS×@fà‹q¿â†ž²)ªÁ¿ç'EÍó¿ëyÎÎÙ~¿æÚÙë'AGNfsrq?ïâNÐâIû?k6å!ê?a..J9a?e¨£TZٖ?Y'éÖVd?[Â]Ç©?ïÉ
j3œÝ?z]âe¢1?hš¥FAÌ?k<Ýe)?nZð~®ñ?q`'g?íè× ÷m?¢chµ?L?£+´G4§?œ*óÙ?œ§œsq?–6Bf"Ïÿ?ïçþªÑ‹Š?w0ã¡÷Hc?9©"˜<?V2"ó¼>?dÌ4£Ú?v?Úƒi7?ïô®X™$?Wà/æ,±?Bu!?̘¯?M?Y*|±?JÑ}_øö8?I'nô¹"?ïæçåEÙ?t"6—~ÿÀ?VŒÑ‰ìô?c–ÞÌÿ ?]g E­Ð³?hj‡$ž.?íÜø®Iv?£?GEgQï?§¿›x `
? ÿÙ> #Ì?"ÿ)ö†u?"t‹Ԍi?ïü¨Qî4Q?B¡ã¨É=?!ÖCGNZ?,0W–«ÜÊ?1Òb¬ÄœQ?AF6‡uIAGN3FGL J1332.6-1256@sãÛ6†¥@HZ3à\÷À8bÒ°+¬À;eä`gI?ä¼èù©#Ð@Å;'þÿ@V&o¼{¿àí)†°¿çøÛPž(¿äÑ~XºE¿ãR—K$…_AGNfsrq?ïø×&de'?I ù6œ?3·ÓKkñ?3úÉûiÝl?BÇ}‹X"t?E¯wzñã?ïºï¹¥—n?‡äRYÑó÷?p'—±Lg±?ƒX)'rp?r‹Z롸?u2""»i?îÛñ3oªC?ãý}à#Ã?ŒsRvßM?ƒq
`Ùm?–H0_2.j?ˆ˜ÃÏ°Ô_?êuÃë?'ÚÊۖ?Bî!x?D7)	>?†ø­6•¤~?æŸ¿uË?ïü¥¾»?Ea–gôҙ?%¼}Ãh?%^o̦?/è݆œ?Dš¨øc²?ïå꺕ßó?i–—/SÏ?WõðbGZ?W(üޘhJ?\4šiâŽ?bn§þì?ïvjì÷©^?'Sì¥Õô?|KŒð7»Ñ?tÝ{í'?"?~9{ª¦?yº?a€×¹?ïë?\rMª#?4$†¿'æî?*ž•>a]œ?bkaVíܗ?[Ïo²GñAGN3FGL J1332.8+2723@Bzòà\̊@T3
ç»À9ÛO
)N®À;꽉b걿ôËvh'¸@;ˆrTÜ%@	4 ›–t¿âÓšj\¿á%$!rk'¿åªøm©?™¿ì­Hœ•¼.AGNfsrq?ï¸Ø²šWÁ?™ºR‰«3!?z-⾝?•"sߜ?bˉN:G?tÓ|$Lë?ï_Ç/ß_?¡šÇM#LË?kg—=@á?r¨±Ð?{?š'-øS?¡a™³ÎW?í?B""‡?¤°rB†Ä?¡™º™ÌøÊ?'쏑¬0?ªr6žJú?£
ñĪž¸?ïæ/æ2àŽ?h@`aLr¶?B	ÕIuâ?Suëd˅G?eMÒZ
?e˜´€~?ï§al<ÐQ?¡MÓåK®?V¯Ô6·?›‹xý>p?cCՑCï?Têv)Ÿ°?ïÍõ/^?Œ"v{cL?Y'gyü ?Y¯S8bý?r¤àŒ¬¨?‹E§#üѦ?íòÒ½Iš?¡´p)p­5?˜Õ§ f"?‹FB
ÆŸ?¤gòמC? O¡4åÝ6?ïüp®/ö?@‹°kÐÛ?ÚX	¼iC?%‰ªŽcâ?9.¸÷ñ$??	Ÿ5ŠAGN3FGL J1333.7+5057@ZÉâ!ȧ¤@P7?úÁÓÀ9PaAcwŸÀ;Çñf	IUÀ"€`¯î@wڿԖÆ@øA?ep¿ãóõ@Œ¿èb+êG9®¿áïZ|ÖÉ¿è(qcDžAGNfsrq?ïýßÔ¼Zd?-'dÑÞ?@K"›Ÿ0?#>iû^{·?(bš$T¦?"P ûvý?ïÃöÝÊÿv?|î;Ðò;"?hl ëU¦?i^´s>*þ?q΀¢Ì?tµ6¿ïîŠ?ïXÍ:Žz?|ž_uâ'x?yu'».'?mgb5¼fÙ?@ËMûôH?u÷"\¯?ï÷ù«@?X‹.?Qþ>숅ÔHÅ?£BzÀSD?Q'ü}Þ·å?X"å‡Åˆ?ïþ±^1c¥?0¥uVü¯?è¨IßI?.C½Ù¡Lu?땚¨Ì?âLÀ\ô?ïêL3J?cÀU´0‡?S"™¼°ô?T¹g:,éÆ?Wã)›/÷å?YGÓ}?ﯫ‰†&?p<á§	L»?oæ^å,ÛÑ?jõe|A~)?x7²ù*'?^éøiü"œ?ïþ³€5?5{Ïf¬{>¯ÂÍ G"Þ>¿-É#½Y?$®Ã5k!?5y
K*Š®AGN3FGL J1335.4-2949@s£àGÓÔ@@
%`ÙRÀ:mOŽ´À;¼Þ&'d¿ßÒkLª'±@iŠ}qð³@_Õ¬˜¥?ݟVg?Õ-¿èjmÜýF'¿ÅxÀtézÇ¿åm›?rAøAGNbll?ïú±¨óÃu?@yŒÐÕ?#îlŸ
Z ?)'H!"½À?@=Àá
½A?<eÉ~ ÿi?ï"õƞ½ù?ŒTUÍŸ?wûcrõ?'wlbôªÙ?~÷ž$?'õ…iÀ×?ï<éú?")Km±=?ÏG¯£½{?uУP¼'ë?	=ÕôIÜ?}Q½~Òv6?ï¡¿ï?'Ž!¿Ž
?VgrÊá±Õ?WN^@4È?%Pð©
?'>ƒ¥9Ö~?ïý°"d²?3•©¿¶—Ú?'ŽÓP¢ú?
éx+/©?*cî€z,?2\-kòHÄ?ïڈTLÞU?lè'¥™?_év»C¡?V
¸'Ð?e'ðy<t?gbs5)t?ïðbËs©?€À…"=?z?à*Р°?wý¹œHìr?~ÇîpÕbð?uö»f¨•ˆ?ïÑ&CFã?kU™¹áÎ?FZȟdp?:"܃Ç,"?t©"©îå÷?j2ºèøÀ.AGN3FGL J1337.6-1257@t_¿ƒ8.@H/öÿ¦=íÀ8Ȃ•ùÀ;G2¼î¥?÷,\Tiº@l"o^Æ@À
2ˆéH¿åCvè@v¿åÍÎ{½Ty¿é>S-¿ãù;tíŠ)AGNfsrq?ïÑ>܉®??ˆ¯Ym†Jš?fU¦¥ó¦u?rÁ?qmú?hk|Å_Z'?€JF
k#–?ï4£Mw'?š•
ª;?Š[Ï2z?Ýñ†lJ"?ˆ{]ž,?'€~6R?îmÁÎZÛ2?,óœýù¬?™È5""Î?"]=6±?˜'Ñ6þ?jF£[?êKú™(?²Ü4M(kž?¸®ÕÄi;?°²
R?¶ PøÚ	?ª'ôÑÞ
‹?¥H
?¼ÁÌAü=—?chê?°Ýe"Úï?zåžwö@ï?¬F'Ž!/>?ï­ê·…ˆ?ˆäÎ="ý?v;]Óâ—?'m·BÀҕ?rÏF…½?yÞ°y—â?ïW^o2N?†ÁœV³!?ˆêµ@@z?€óõ‡xò?=®ôa½?wŸTîÀ¥?í™y\%'?"¹'j?«c¾Rvõt?–¹þ4?–	QLÆØ?h_æ "AGN3FGL J1338.6-2403@sÉ}sÉ@BÈ?`h¤À9£ó=yÞÀ;¦Ñb§•?҂Ez2¡@¾]c2Y@œGÿsF¿çoP@ñx¿å6ÎDŠã7¿ê,øËG*¿çïs
q`HAGNbcu?ïתÆER?l
BÝñõ?o}g͂I?iL
mŠÓž?RçÛ5æ)â?OõPqŸs?î?%´tˆ?±¦»WcÑý?ž×Š‰éõ¾?ª®€'¢ä£?™C¾ö¿GP?¢)] ¶f«?î®ê¯òݔ?zêΐ?zF¤ô?q\6E¥?™¨cöoi?…Š"?¨ç‰?êRãCÔ©?«qÂVz€½?¸ÔÚL)?¦âfÔP?µg]i	?£íT§ƒ?ïóïœÌ ?Qgú
ج?QÚÌH|H`?Mµ‹â°ê?9sߢ?5·Êµ¨2?ïˆqßIÞ?'j·Ý;)Ù?€•LIî­?‰ø³dÙ¹é?zœx/Š[â?"µ¸Nµ?ïqkčj?wp¿i?€¿ž¯…x?o2úl?'åøq6
?k''š¸"Â?îºüôÃòð?Š%IÅî?•wRïQŒ.?{c4gñ—ç?")MÒ?ƒ•ì®¾AGN3FGL J1338.9+6532@\Êοìº@InßÜt
À:"H¶R7À<$LaØb,?Ðуüàw@K–ä³s_@(·_þs¿é~+Ž›†%¿ê…ˆ·bò¿ê¼`ºAÛ¿ïû˜Ì·ušAGNfsrq?ïAéšôôš?½ ˆm™­Þ?—g'•¬@?½#DÜ0 ?Eì¡"ó6?Dúƒ8WK@?í"YSXl©?¬—/Pãbß?¨­÷Sù'?£Iˆ1M?žæçç@¨?¡$Ôm!ç?î#`‡ª-æ?–"Ü"‹ªÓ?¡‹AE˜›?'þð²ñ_?˜}lÚwCÿ?‡3¤Xuž#?ꗻš9@'?±{]b×q´?ÁDÅ?¬Ï_¦¾!7?¢C5뼌? 0ðÃ	)?íy"zyKy?Ϻ;M'‹â?´"ïëH?Ͻz›òh?9ß;¾ª??ùå?ï`4ÚO†?‹Ÿn%'Û?ˆ²-àÐõ?ƒÔ¥tŽ?~ÔSóRä?~b8•Ûçw?îÎw"\‡?' ÒÓ4?šËÕѺ9¦?~ý›}ž?†ä¶šÓ¢Ì?vhŠ¢ï¥]?ï/ÈtùQ:?‹ÅåÍ°¿©?"L::?w0â@¿r?wê•1@nú?~§÷±w
ØAGN3FGL J1339.0+1153@uWŠ?‰'Ë@QÇ€Æ^À9ž}þ2 fÀ;™5<ø®Ó¿Ø{x´û'‡@ªtb¨kÄ?ÿrKl÷¿ÑÙ¸K>~¿ç•èµó¿Ùͳ¥g
Ú¿»û¼WgdAGNbll?ïç>cE¨3?``Q*hT?BæêUY?>¤&=·(?d¢ÑqdV?]L‡
?Ÿ?ï¼f|z"´?€°-Ãù?lä°Ä݂æ?qàXV™ ?sZi'£|}?tÌd…'0?ï<G#š?ˆ_i@72?‡¦VSdO7?ykX\›3
?"%RMie*?äÛü[€è?ï=´©?~ñ?Z­u™Š*?K†j2m¬.?S<ÐXYÁ?—m7o­í?#p@±€S?ïöb†'?HÃàÑ®"?4ûYÑËR?0*"ÇèR<?M2£J?DÉìvB@?ïçJ¿ìÀ?eÙÞª2:?V:MÙÿœ¢?Xrž`YX?[›)dp?['éþª(?ï‹c.‰¼h?täjV飯?y¼ G6Œ?lÉÿ_Àˆ²?€I2]†º?i D@ê0?ïÞâ¾Ý˜?d:'1U?3…ÊÝK¹[?,c7MÅ=á?n­>ÖÄ6??c¼knvŸÖAGN3FGL J1339.8-0133@to׿¤Æ@M"dŸ¼ÉJÀ:$5a
ÜÓÀ;Ƽ楻ç?JQÝÃ@÷«yjúö@À	Às"7¿Þ£j?^ÿ¿æ(wS¯¼¿ê¥Xl~¿ïÿÒ~ù–kAGNfsrq?ïåYp´ž?iší¡ï•?bx ÷Í?b÷á›sØ?Q."}?T%·a»Ú?í-oOÌ¥?³vX—ˆØ?­-wÌ°Á?®®[®? Ǘ'ð?Ÿ›dPà¸Õ?íbó…`¹?£@1²2J?ªQ߁›?œRZ¿	ì?žýò`d¥?'SEkž ?ç@?9yì?¶M\–Ñ4³?Ì:4ÞrÖP?µõª+ÄQ?«;Q…?¡j|yççI?ïòf›%Æõ?W¼üD'
?Rš½0y¦Ô?S¥äëÑo?A00³Ï?@X¸R`{?ï.ÖN£?–ú€"õÚT?"<¤Øe$?"3¶|4?…;®'þd?•÷Ð:þI?îÀ˜Œ†ê?'÷ØKJm?šº)ý—?ŠüЛoyä?‹¬hƒkÃ?lxùƒ?í$šÉó:?šÐsåâ¿?³ªPû4*?–˜™!K?Ÿ?‰†Ô:ÂX1?…œ,LãS9AGN3FGL J1340.6+4412@XÀ`#@Qz¾zÀ:'k¢ŠÀ;â;Ñgf?æ«S	@
˨/3Ÿ??þòŽ?žPŽ¿èVŽjø'™¿èè¼J&G¿ß-Ñîäh?®lª‰gAGNbll?ïí5gb\8?aš€"a§?7-°Ê³!?4TT»1Ã?_ÉÅU'D?`Ømœˆ?ï°#6_?‰-Rþ½{D?r"Æ›&Ú?ƒGl‹ à?uèà#¢¹¬?xÖýÙ±K
?îøÊAé@?"Þ'YúÁS?"Ša²w¶?q(ÿԒ8.?–·uàrj,?PFí	æ+?ïX5_¢Ù?'Åhùjnò?p'âË#mÛ?‡9£çZªŒ?ï[Xpxq?Œïˆ3"÷?ïùc²h-Í?D±^–¼4?'ͨ
Ðl? 4^?.?D}ÌDd=ó?C("=m*?ïä:æ…Û?kã=êÆ?Yo<¶Æ?\œGBº‡Ì?]Ílâ?b†Aei?ï€2ôˆ?yÛë–AŽ?vØÃX!ã?bj¸¢ÆÇ?"'¹Önð?v3LRÿÚS?ïÜúbÃTå?pò¢xÖ›?^q%@[+Ì?dÑ¡x®8?cÍ
з"·?dÂe .^cAGN3FGL J1340.6-0408@tYæ?šIÃ@LF}À?`À:¨nH²÷À;®Ù1_?Õ«j¿¸¬@Œˆ;Î7[?ÿ³»@³Nw?Û#8¥fŠ¿ÒXlŽÚ´þ¿ãÔӍêí¿âˆe邩ØAGNbcu?ïúPb»X~?@-*·¹í.?5im×?5=2ÌûÉ?8}vµ?0ÒÉH+e{?ï_ýÇý–T?–ÌdÆHç4?ƒÍš1­—?%Ãtcž?"2Ë_‰…T?ŒÄvëJ»?ïR³Æìc?;ŠI5š?…ÞxXÇ»?w†_áU0?†;/É×?s'7¶ªÀk?í0v†UUX? À|"k°'?¤|í»ÐÖ?•ƒ±wr-?¨{Ó¤?špv&ü,Ý?ïý…'À?/%ók<P?#÷«T³?%6e>¤î?#·¶Äk²?î‡ÎCä?ïÍ\dãb?wû+²Cà.?i$Ǹ£cŠ?j$1Ë֟?i~ÓXûÄZ?p@CŒ"?³gå±?rî׳ž?y$øL|å?nƒGÿFô?všpbV?_FÛ;dø?ïM±îÇjÛ?'¸óÁ>?‡\=ÙKs?p´¿µ™É?…7GNz	Ò?}<)æ&9ÎAGN3FGL J1341.0+3955@UÑ¿íÁ9@Re¢åx•À:o±,]VÀ<ØúØy?×'þøn@Ÿß…65F@Th€Z¿èôԏ}¥·¿èÓ¾šžÁ¿ÕQ8i'û¿å|i‰'ÿAGNbll?ïø€hVfÐ?H‹|ª×?28ûuóƒù?7¶+¹CRà?DáßæH®Ç?C:£\îoî?ïyàk»
?‹Ö!G=û:?€RQû°?JGÿúrâ?'³9ël?'[|"i]?îÔːP‰t?U5#"Ò?‡§ÌãD?u<š,Áõó?™'§8Ùá?†U'	«›?î÷
úæ?–¦Hyw'q?‹­IÿÇXÁ?ÿ"N5?"GYTðî?‹^Ád5u?ïü|ŒåÎs?87	¢ž?%¥!ΕÜI?0¬ÍÞÿÒC?1I	$·R´?,cјÃ?ïÑhCq€?qýB@*]?g+m>¹M?g¸T8ʆ?glO`DÌ(?d·¶8i?ïˆKDÂt?r®û]˜?wüú»í?c´è©í¾?'fîÏë‹
?h÷عŸu?ï»%¢üÄ·?sš"#žœ?xfÂåj?i?Ô:"'C?dÔ.2õÎ?f&àodAGN3FGL J1341.5+5517@[ú?̞ª@N3·ßÕ¾
À:aLç9`À<úˆ²Â¿Ç½²"¼¶@
s		i
[@ ^š?¿ä1æ×åÛ¿ì¥/`¯‡¿Óƒ¦K6gÏ¿â«}Ww=ØAGNbll?ïâg^3?oÖß9Ô¿?+'ê6?)ˆÞ—9y?lNO¼©Z¬?nþ"Úm›?™·v¤?'ã%‹Í?}F«Ÿ¦?†À¾.uõ€?œòæ¢?…¿öus¼¿?íêÊÂÊÚ?–ï+'(Â?]',mT?{:¯°/©?©$–›å·?"á+D–S?ï/r#]þ
?ŽL/Õñé±?oÞÁˆuUÕ?pk™¨žt?–ã^b«?‹¢!²˜?ïó!uϳ?rý€—쥘?"Órn8G?7ŒI²×Ý?Wb¦uœó?q¥0ÏÌ?ïڐ:'÷ž?sÇæ±îÛ±?ac¤ÐÕ?d·RݵŒÆ?d!"à©?hµÿˆSÓ?ï8¶È·?ßðÐe.?}—Ïm?gYôbôß?'ˆUZ—©"?FoW?ïÖk•
Õ?k\|È"?\÷ðIÑ¿?N‡Ã˜eÉ?krÁ¬Eã?fàkKc¼ÏAGN3FGL J1341.9-2053@sèàm"@D8ڿԖÆÀ9˜c8´|À;13~²Ž?ëÊ]ð‡MM@-ÍX7úm@/òä¼®¿ã6¢Âž[Ü¿èý,Ñø¹B¿ê˜5ôâJ¿ïÿxÓ·‰AGNfsrq?ï÷nOO.Î?I2ný?Œ_?D…ºéT´?A%/ã‹?;'WDáË?:Êx6Ú÷?ï"䮝?ŠYy¾¾ßR?yw}ෂ'?tòÌsI°?'9Gàñr?…¿EQx*¥?î»ÔTU—·?[ª›€–Â?˜Æ:"Mü?‡üo Îvƒ?~uÊß8?'">½?ïV'Ž
Â?/@€ê5?€ÁÅô÷§W?|  dÎr?‰™óãe`D?‹­ÿ	ÈÇ?ïøÑ<óü<?\XíNÆæE?F‰θ%?[à5p‹i'?(È,5ßQ1?$CxÜ'?ïԒñV;m?n#}yxŸø?cí5–›}–?\fK7-¸#?gÙ'Ôù?fw•Ø~»?ï)á³8Ò?ƒMøc¯ùí?'w¸'·?})L©xu?ƒ\£²Òü?qÔۑÇ\?ïÝuTHŠ;?ijÙUÜ×b?aèáu\?VY€]^.!?aÂÓAž?dü–+äAGN3FGL J1342.7+0945@uCoÀL‹Ê@Q5ÅÑqwÀ:a±…H©½À;¿¤àõx¾?ã¤.)wâT@	L˜ Ë<)?ýë8$®¿ïý:]L•?ïàü¬äO¿ã=ô¤"Y¿Ü±z>"AGNbcu?ïðéûq?fM)}Ο!?@Ÿè×@¿?<U4»1J1?UÝßFß{é?f`™K4C?é*ÈÜIº?ÌÚ|&°Þ?ÄŀÝàñG?È£!"߬Š?ªH¯ÿ"A?°Ò«qÓïæ?îæ|7wÕ=?"Œ•è´€?ŠWQ/#'\?xè~œk?–ÐtL-*?|~–«J•?Øæ6°–5a?Çì	öEc"?âXÝTŒý²?Éñ!›ƒ?£@u46GÎ?£FxÄôó?ïñû勁ö?'_Ü(žP?*Nñ¢j¼?&'¥÷ÝZ?X¾Vë[ǔ?'cÈ~Ý?î[nAL?¶h™0•?£‡X'v|?³€j¦$?‹´#'2?"²+HɖŽ?ïoÄ©Æ@?v@ÑAÖ®?~Þ\õ¬óq?q!ã[«?"Ÿ§á°³?h¡KŸO¸è?èÐ .H½´?¶ò\*,·4?ÊkÁœ9~s?¶x}_ê/æ?'íOôëí?‹…îSö›TMIXED3FGL J1343.6+5753@[xš^»w:@Lñ€@,?úÀ:ÄNÁ.3À<rãLk¿Â»ëˆÏœá@
ÁRæVáŽ@C1¿j¹‡¿ë&n"å¿ëRf¦¿­L‰×•ä¿¿à¢ø*H¨æAGNfsrq?ï‹ë×1³4?¡JærÚî?U¬«ùOX?bmõ‹?ŠOt²Y"? ÙÄTsÃÉ?李h´¹?ƒ×üç€Üü?sšPÔ#ó@?tˆÒâ|?x"ú´¢Å£?}žtÓ|ì?í61ú<áL?¡\F%&¡?™"9ý?'Ú¤3£?°á®Ø±b?žØ¬¾ŠJä?ïœØitI?'ÅqÑÊ?T¢~1·X?_…*9£?†5•ì™yl?µdûÖ\?î媁s]?À¤i_m_?d¨w· ?}	AÒp@? ZÏÕüÝr?¿dñ …ŠÞ?ïßèTßø›?lÌ[5wZ{?^{^A©?_<7ÞO–j?`Ùû¸‹_å?`ý¾^Vk×?îç·c¦dû?GE•´¨V?…ìIM?€rL¨Äº?˜
-\Wå?‹ªº	mëU?ïíÐkÎìH?Z+[xv´<?Iiü5Ƚ?DP5rã¢?Wª*ÎÇ6(?Tf8ðÁ²AGN3FGL J1344.2-1724@t?Ÿ‡ð$@EՉ?¯BxÀ8ICÝOÒÀ;+ÔÏЍL?÷åKà¤@nŠ§ŽNã?ÿqZÜg¿ÛV×R6Ú¿âÅ¢¦Þ{¡¿âЬkêp¿æ΂&é²AGNfsrq?ïùc˒?Dää¦÷:á?4†ù(ªý?2îªÉpÂU?@.~ÍÎE?ABê©'!?ï—ې?Ž‰|œÜå·?v4œ¨aoq?ƒë¶ºµ]?~IÖԈ»ú?ƒb‡èvá[?î³ü3—²?•v¯jÙk*?'ò¿½ª ú?‰çƒØU)?—¹ÑkI?ÅÍá*ß?ïy­Àíñ?˜$%]¹lé?{cvç!ë˜?}sàÕöÊ«?•wìŒ
ñ?•ú(ÏhD?ïüéFøYe?.qc1ƒI?+,'Œx?$sÈ"âW?&>ÿP,?!	poLý?ïÜØ úÓ?nùá#?`Š¾Çm?[+'ä\Ö?bÂVOå•?f×6OÕ?ï¡W~0?'ö%YØmÓ?‰­g3i?'µ/CàŽ?•
ZëåÀ?¨Ì+V	?ïºôìQw?v®•[¾~?q@÷#0o?dm˜=‡Í¥?qD'è5Å?sh˜ @lAGN3FGL J1344.5-3655@s©[ߏG0@8½¿jäzÀ:'‰)ßÍ[À;¡µç­ù£¿îjÐ;þD$@
ès(ö@t{ \ÁÍ¿Ûêj3œÜç¿â,¦|+½¿ê\Yf,? ÄNE³aAGNbcu?ïÓç:X¸Ë?q8Š2Mü?c}±ƒà'¯?bí¯ƒVZV?h›/Å:?h©¶Ç Á9?ï¯
'°°?ƒÍPàØu?p%ҐŸ»?p5 ˆ2¬a?xSl˜•qÇ?€!Š‰G1?íû/Äéè?—þÄTp?œqƒPTÏ?Ž{:쌜
?¢A핂#?‹Ö'åo¸?ïyáîЋQ?ˆÅ:¼|c!?:¿CÄã©?F¦°Ošæ?X·0–;d?ˆŠæªAÓ!?ïïªÈ@ ,?Z]'õÔ¡?H°LK2??K¥Ç0"'?TRIˆ?S‡ÊöD%°?ïâ ©áÃÝ?e¹©:v?Xh-œ3'€?RëFfæÇ?a+?Œ›xÿ?`µµy·
 ?ï0×qI!?""­Â2¤t?ˆÿâÓé.?yÿ1v›4?ŠÊ@ÒïUØ?wp»ÄÈ:?ïês6›f?\V7_A?³îQ6à?
ƒE'>IH?eú:X•g?\&ÒGÐ%AGN3FGL J1345.1-6224@sQş±á¿ÇõS`œšLÀ7À'°H1ÈÀ:1È\$Ä?óH•$êÆ@Ctà&Ç@É'?_‡¿ÙY4å
å¿çJ'QžX¿è'}Ô¿îßé	Cu¡OTHERspp?"}¼¥T';?}—fÆ)
ã?×q­E·³û?ËqYÉõ×Þ?ãõ2jœ'.?˅+U²ÿ?p÷\ßÔ7?€·Åg÷_Æ?Ö¬àaޟ?¿ª‹Ú>Oq?ä‰uáçÐ?À,#ü
$?´Í¬Â? ÐA¼Üì_?Õfÿ˜?·ËB%lá?â²øõ8•?·eÐ0²å?°×cŠ?S>#MÎD?Õ0ݓ¡?µcݎgÁ˜?ãL¤Ö0F?¶Ó3/åó?~ÒF1³Cs?{~î ñ¢?ÚÍ2·§"?ÍQ®åAsú?â[Â=äg?ÍmO÷ªO?'C¢sµ=?—ž¡n?Ú¯´ãn?º;ÝfÕw?â^0±g…d?¼ÎH"´:?ÂîY±Ä€?«ti9xžW?Ö`
{?³'pî³/ ?àh
<?µ³P.Á‰x?»êxµ.²?§k±&n¢Í?ÓìT‡8?«ý']y?⌥D?Ž?±l?gã­ÔOTHER3FGL J1345.6+4453@WÆ"?@QL`×óÀ7\ahФÀ;|7‰?ô¼
?Ê5@ b¼bÇ@×kŠ½‰¿àš§*s=‡¿åŠÛyŸŠ¿ä¹v?¹¿çwi^WAGNfsrq?ïùúנּ?=àoÁ¹k?0î§M#€?-‹Ԇ,«??@oi¸¥?7_™ŠÇßa?ïÈí¯›cž?†'¬úñäŽ?k¢/?]¹?':q|*Y+?l®Iú«õ?qJ/'¥«_?ïY/L&|Ê?ˆRëpï?iC¶ô(r?z‰mѤ)?ˆJéECû?'ǵ~¯
?ïüTB?V~\ÐÞ"ä>ê`tt*?Ɉ¤¯p?>섏G܈?Vt>5B?ïüêrئ?,rŒöʚÜ?'¨nD²r?!'—\²n?)°ozàf ?!û¾{–<?ïëY¼x°…?fõþ1q?RoV¥UE÷?SÜâ@"×%?VÝ0w "?_,BšVd?ï‰Ã|&?'5'Ÿ»e?zÃVW€¿‹?sAáç.*?€Y£ä»öÐ?z¨ú†Øš‹?ïÿŒ)è?)
tÂH×Y>Б'ßºf>߯(;®Ã?
è;àQ"?(ÛΕ»¶7AGN3FGL J1345.8+0704@u# ¤<@P‰Î€+3ŠÀ9gíO#À;™x'â3?ê·«ZŒ='@øh‹Ô¡@z¥_ö_ÿڑ]ÈÞ¿ã³MŸ<"&¿ç­Dõä"`¿é†e¨Y®AGNfsrq?ïëlÏÙi
?ajâ!tÑ?a‹‰~uÿ?`F°?¯·£?8=5çq`?1ü¢Æãõé?ï«ò"áp7?‰enеh?s=²ìñX?ƒ-j]+5?vÉ<‰È)?{wtªó›Z?îY>Зª?šîXƒfá½? _†}|m?•ÃB4'é?" K1Ô#Þ?‡ô¨~¦Þƒ?ï]Î]Š?Ž$Ý~!£Q?€ö׋5^?{*Ï1bö?ˆx…'ç@?ˆ­æ´}Á9?ïöqÃ*¦a?OÆ94Ôóã?PgtlC'?N+2^öH}?%¨(Ñ'? ½~ª‰?ïÞ¨UãÑ?m/Û<·£h?[òOÑ(X?WáZ€XšÁ?c^'*ôÌ?f|)5tQD?ïUIÏà[?"üàc¼ð?Š•týËã?¥&úm?€"¸•I?r•b~:?ïÜ¥²×ƒ4?hв1ƒlD?c—ã.ã–?S~6¬ÜaÖ?`RµW+à*?dŸ'ÚKN'AGN3FGL J1345.9-3357@sºÎ wm@;ÊÀƒoÀ9Ý7iù˜ÞÀ;°¨YOý¿å$Ú#'Cy@.¯KÝy@ºs 
Ìã¿çvE`Ô£}¿è…ù‡¿ÞLs'·K~¿æ
z'R*AGNbcu?ïð¸ú²ä?[)§<3Ì?:œÔŠ3™H?3%þ#'h¢?WæՄOß'?X¢µ
ö³/?ï"Ø€Îá>?iã<ˆ™?vèT= ?'Ѓ/[ͅ?×L'Uä?ƒè9ËÖh?îá'xk3?º½Šø\—?ƒ1£•3Áî?oS0b£1?š4ÿ(N.µ?‰•È¤€Ä?ï;J¹8¼?†Ž¥àÿӘ?VtP^8,?QOkÒ#âR?—.'"»¯?…Äk¯o|Œ?ïüI ³?:¦aº<?$YÉûþÙ? 
Ûò™5?3†~Pfð?6FR@«?ïÜ:Z™Ô?k‰ý\q þ?^¤žv«?R…óà
!¡?dáób~H‡?f•A§1‹'?ï'ãVùP?uIJÉí<a?sfÝ(íc‹?b
Ußø§?"»ã3T5?rÍŒÔ53?ï׈Òy?cEíÓã+†?@	6eˆ	b?.Ǒ­?r:É Œ˜Ð?bz"ŽÎ¤AGN3FGL J1346.6-6027@sZýq??ûSA§vÀ8j^IarâÀ:ˆuk¼ç|¿ÖÈ,
=ïé@ƒë²k"@‹C…¶ä¿éªÊ®Ô-¿â7Bvòû‹¿âÐ=õÙá]¿å<'íØáAGNrdg?×3šù¸_¥?Î̆ ‡?£ƒ8‰R\k?¦ètùŒ?ã-þúW°§?Ð)þ!"¶l?Ȳ'Ș?ÈROb5?µ·P¨ëÅV?±W@SŽ9Ã?玆kŸ?ÉQ¼úáví?Ùȸ`Y1?º²1ý?Á+¦!r™?«•Ž*«&?Ý¡t•?¸©he6i?ßëö€ç?¿ˆèÓH×?'¶î©ð?"çà#–³
?ßɳª^ZK?¿Í±†ÒL?åOn>ïKt?І­S_Îr?–h㜱¡Ú?™:>ËX3?Óú•HHº?ÐGGa|G?ØÑÏ®²
6?ҕ•њ+?³i\4ë6s?¦9sð
ì"?á)ì¢w†?ÑZñ™œ?æeØ¡c´Ó?¶
õȝ?´¥uWáb?¡8Œàúâ?ÌdJÀ¡#?³k¤‰×Ð?å€fJje?·×Û	*À?…jÛßòëÜ?sÒÏi·d?Õ1¨SƦ˜?¶èC/ÉMIXED3FGL J1346.9-2958@sÐe`A‰7@?_ð€0<À9»éœç+ôÀ;_šÛ¸øÚ¿é'©jz¥Á@œ¨žoAV?û熿wNÁ?çKÑ Ø8¿áµ¤g¡¿ÏUsã/Bk¿Ö¨xÊ/þAGNbcu?ïî#ùHD¬?WóÆØf?F C¡j¹Å?DÕ³ó"i?XgëHþ>'?Qº#f/^?ïŸZD³Òð?‹gõ…ô8?s'•vñºG?'2ÆÄN<?|ÁH¦®?s7ºÁY?îý¬"T¶?…ç-«ù¦?Š%±ÙP?w¾­—±ù?"	èÔBÌ~?~Ÿ<ÆWÜA?î_1â-åŸ?–Ï[§Ž?HÝÙâ:ßÌ?J-nìîØå?©©jvZ>)?–¥žÇjø?ï÷ès¾¶?A`Å<êYÁ?4õÙ^"×?.½^ÿw?EãDÒîƒ?;7ÅÃƚ?ïÞw(D["?ms¥ôm?[|ùü^ùs?S¶€†Ø^Â?cÊZ›Ø?gæ
ˆ î?ïÝRÎP?töSÕÿI?~÷¦$Ïe¬?nȕ.Ÿ«z?€<õž¼?d}þÏþb?ò¼?tÇñ9t[?5bïÄô3?(üŠAYÈ?Š$ëüû¯2?tž͛"AGN3FGL J1347.6-3754@s°>€8Ÿ"@7¥`/ÁÀ9‡"ßöÀ;l³X‡€'¿ññ­w6@rš²t@ñˆŸ¡EŠ¿ä«‹3؛¿çt½ÛB[¿âû¾ŒdŸ3¿í]0©"âíAGNfsrq?ïöÈF³Ì(?JX³gÙ/r?@Š>%ôÒ¨?;¯Éš€$?DT¦3æ0?Aäk
?ºz?ï²DY\xã?ˆð_B›¤?pI%ƒâ>?'KrÉ9?v"­çþX??}}æ÷L¨|?îʪ=€¿?'M}µƒ?"â…ʍL?‡;¦ˆæ$)?'È2…Ï'n?ƒ¸ÿâ!;?ïÄSÐüK.?x÷¯ìB¼?0ÖZ]³ò?>':yÏ?|È·]\¤?xƒÄ	ušÅ?ïù×;³ë?Aä¨ï1`?AZøÐA£)?=µ2]g' ?- e®rº³?(×X^"Â?ïßWÎ^Ù?h­äJ¤ä?Z"€ïã6?UMÝ(³º?c_)0§ôð?bÕ¤ƒuÊk?ï*ø4À¸(?ƒBþ¶‹Ž/?v¯?æMf?}ÐU¬PŸ?"T">Y_?t!N¯'‹¨?ïôl,½¼þ?SGÒuâ?__ÄýK?-Ûv6ðã?V4«A>Õ?RÖK—*ˆAGN3FGL J1349.6-1133@tNßÒc@HhŒŸ¶MÀ8¶ÐE®À;mÖ£æ#¶?éJ½ŸCÛ@Ûç3€`
@"³Gùi¿ãÒ©p&X¯¿äQª¶2½©¿æúC‰Rà´¿êh)pMJAGNfsrq?ïò?ø_ï÷?V̟š€oŠ?W÷N@Uá®?UÌĸ
?,Fӟ¦r?%9,7f¬±?ïÂÂ/Ãp?~†Ÿ‰x/V?k:è‰@Ü?m\/g¶òj?q~"WÇ¡?uB|X?Ÿ?î‡4RJ®-?–÷[ˆë5>?Ÿ>µv¥ì?" IbÔÉ?¶Þ•4å?DÄ«m8?ïð[úŸ?dÆÏ-_j?)Ž½ê'¡?@·ŒÈH™?\4"¾4ð?c•ŒFÝM?ï÷<ä{®ç?N.'"‹'p?OhWbζ?LêÎФ®–?x3–Ûã?/ß!
µ?ïè "{ûØ?d"žšKÑ~?Vagþå?SPIüpÑì?Y]qÄì?[y'ÔgH?ï\ZףÝ?†²ECd?ŠH¶=DÅ?ƒM–îdé6?}A'ýqóŸ?m¨	ïL†?ïýY¨Îüä?=^†"=©(?-÷Xâ>?~!#éù?0§:uίº?;—LY"'AGN3FGL J1350.8+3035@I²Žÿâ£Ï@S#ÏÃøÀ9
˜®¸À;Â^VY?ì÷"úXÔ¶@«[ƒc@ø¿ƒŽ¿ÛPÎWD1¿çŽ8éð7û¿ã5MTÐ'¿êðw2!ÌAGNfsrq?ïø`jtF?E+ž'z9ã?D'úW´ÆÀ?@²ÓFáõ?3õÜÓI?2xՍ^š²?ï´ "ˆÞ`?†£uÚZ{?nÈÆ î߈?t£;	:™3?vKS=§Cé?€'¬œ«ôÇ?îªÑ¢­Ñ?'âÑ 7¸?˜ŽRï…-?Œ ìíP;\?'ۈÊ?'M·?0:Z?ïÒmœe§?v­JÔw)š?['¾"¡ÕÒ?^eRH¤?pِg‡G?tNWKÍP.?ïûþŒžšœ?2síC—Å?8¶ Í"Ý£?.èx€}!#?Uáɾï)?CÌñA?ïÞÒ­Ù¹è?pòžU?Zµ·—9x?X!™t²Ý?d÷@ۓÂ?l°>†Ðu?ïUp÷'Ù?"—Z¥º?ˆ¸<L*ˆ¼?eڇÅæ?''f=M?sÿèß!@?ïõûļ2?TÂF¯dx¥?D
»˜°-?@E$›ò?DeÚ<ð?PÑ£a­ýAGN3FGL J1351.1+0030@tÛz WŽ\@M⟾vÉÀ9ãÔ;kçÀ;»€õ]县ÁRڅ
@'Â("¯@€Z€ª	~¿åò@òŽ}\¿Ýúê
ò©¿å6èR¿îVÁ(ŒëAGNfsrq?ïÀزßð?x…ZñàÒ?}O͌ר?~®#"ã€Î?BÇø¿˜?<¦MHÙä*?ïº!–þ‰³?€†Š-Íæü?n÷ÎÊP5@?rŠ~­\Õ?ssM8oÔ?u([FØ@›?ëêòu¹ü¢?¨-o«?ºr÷2?Üÿ?¦Ê¦
#¡?˜ÕÔsºUà?Š@Dvyw?ïÓ1ø—ù(?q<…Y€*Ü?U—'+"A?ZåÊVÉ8	?qW¿!?néö!Û?ï­	œr"C?†"Y'}aD?ƒÓ'©2ƒS?†2ä¦)Â>?=@åìð"?:JSۗ¬Ò?ïå‡Zãâ?e‡"FBƒÚ?Xø¸Ió=?U™­ëªd?\9†õ­5?]"­–'?ìÏ÷'5­j?¥Þ*1Ä?µ¿‰
ƒ?£ZqÌËö?'¶îvË?ƒË¢O}›&?ï÷É8©ÐÛ?Mà.3ºäj?3|j2˜Ž?9ÈÌǺ³?Go?H22ìڎAGN3FGL J1351.4+1115@u·
?‰'Ë@Q2€	¥›À9rÄÞÁÂÀ;G²'a½?ã£àU§@š0øñBù?û^ƒþý¡?ïõ9µÙ@N¿Ð÷ñ‹"¿ÛuhŒÜF迪ªºaAGNbll?ïâŠHî±N?b/ØHu¡'?_†•¢{?XN¦ç@¬?[dØ
ZYb?S"nN=­ç?ï¢"‰íª?Œg®…§ë?upG!݌?€E#o²z?y~µãY??'&B÷+ß?îÐâ'ÝQ?¸ymOá?&'~k9?'D.J¬Æ?•½"›i,³?"¶{Ý B?ìsç	}Æï?«êR^›+?"vŒ'WÞ?šWAZhVV?·žê[f?©ùŽF<s?ïòl#"·?Q‰{o‡)Y?MP°{™7¤?I:;Žl,?Hþíøãñ˜?@4‰ì•ô¥?ïÝMð4?pL1.À?^!èÌy¹?\bé]ï?cÔ½Õ¸¬£?ió
hõ=)?ïfÿ²0ƒ?~ˈ¾¥Î£?'SlÙÞl?tA™D¸€_?ƒì¢""™¾?u®šåÐ{?ïpq,= ?Qº‰?€[Û$}k?xƒ
Kì?–dQí_I?‰ÂvlàaAGN3FGL J1351.7-2913@sæ³ S\ž@?ӆ?IÁëÀ9}ÁÕ"äÀ;Œù)L)¤?ÙÃp*"2@ôªaâs@+"¿lçà¿ã¡[òï÷¿åã'*È¿ãÆ_׈¿ìHõV±AGNbcu?ïí©ÈZ€?_‹upmÆð?Y=B¼*M?Yjh–NÛå?FàÂd©(´?B.–'D!³?ïIq+*??""n™]+?"{IÁüu?zÖø˜*JV?‰@šœEgá? ^AÅ@h?ï)vÛËå"?†³
dë²®?º7ÿÍù?M߶NP.?‡è,Ù?r]j¦K?íú
ʲ°?—ªh¼'?"mÈ'	R?Ëý_â̽?¦¨Ë!PW?"VÙµÑN5?ïöÄÑðfõ?K€¥ ®Ûa?Kí3qóz*?Gêä›ü‰?1ÿ	ÇYË?+AÆÔ"G!?ﺠ›…F?y'Õ£]¯?pn¬|¾v,?cғÙ6ͧ?rŠNì¼?u)ù.›?ïÓÓYâR?y­,' u?ƒC¥\ø~Ù?u+Ïaà™U?yŽË¹j-?fOÙ?Ì«?ïybí`??xnòËè"?|•œ0À?c`+h«f~?ƒ£yÛ¥åþ?u8î
X:üAGN3FGL J1353.1-4414@s§?Õ%@1>c_Jé2À9YÕ£5#ÎÀ;‡ýgŸKŠ?ÝÅÔGaà½@×Nìő@¿P +"¿é‰–Ü"°¿æåÜ+8‰¿ÝìäÅ<	Æ¿é3ѳ]ÝMAGNbll?BVÍÓ?¤µËìa™v?˜ÿˆùȵ9?›étÃäU[?'ìβƊj?—€±¥°Òf?éøÅ«'·Ê?Ã'›"4n¶?»Â$Aºp?´ŽðR2ÞÂ?´w®bS‡<?¸ˆ‹nýq'?ëò¬åüŸ?¦÷1î?©ä‹BYdø?˜º{ß®á?´ð$øíC
? 7lXèh?æ$ « œ?µÆ™Õ X?Àè"ÁÎʆ?®5 Œ&9\?Ƅù?'³	?±­/ífG?ï§[gôtË?…5¯·tœ?{XŠ—ˆqM?~ÁN¸(?pùÁTÐ
2?u
»;ö?íͬÐÐ^õ?®DÀ‡ñ°Å?£wk¦ªÞ?›‡î‡˜ÌP?Ÿ[Ž–è+¦?¥­pÔ
Û?î…-i1r?¹Ovz?•°…:üœ?†Ä䑈ª¾?™©ÚÖç*?ƒqjÊm?ì*ú³£?¡êo:å?²2H[÷=2?–dT·i¯?ª8¿ O§n?•ÀŽ•b0AGN3FGL J1353.2+1435@v0":¸c@Qº¿ÖDEÀ9ö†º À;Á¹ã»ü›¿îy­:@Öç,õW@½œÛ½€¿ã.êiž\Õ¿è%ž8uùh¿âr2¹«¿ÞЮ›UÓ¾AGNbll?ïñfµËï?eŒÜU?=Ø[@1
?IáÏI"?Ö?U¼~ùí°µ?cÏ>·ß?ï¿b>l*?€_a¿˜?l{^-zg?rŸd¬ÎdÝ?rŸÖkOc?u4vš].D?î©ÆYÛ?—XéKÁ×?"Z7o]$?ƒ¦-ɸU|? WдS}W?"ë—ód+È?ï¯Eú—r?|‰.à??Äo-æ?>L® ˆÝ"?ƒ0›¿"È,?{µ=Štð?ïûŒåoõ ?C
':r5¤?*؆-ôâm?2/z€åâ?6,ðfN¥??N¶…óª?ïæ8ð¦4¡?ez2Ǎ¨·?Wr.Å27?UX °S4O?\ïÝæ€?]M&ÛSPÊ?ï]›]'ÖÎ?Šè—»q0?{ƽJðˆ?:‹:\ýo?ŠµÉûâ(?…™YYü?ïôòÖÕAï?M­IÞ,ð?lA†Ö ?	KŠð0Zþ?T³Ž©Ø
?M&7W–AGN3FGL J1353.5-6640@sP @|ÇÒÀ#7À5º¢À9]ÇËÜÀ;BЉï•?¿˜à«ù@œuÁù	?þ{``½Úì?¶Ú¡Ì˜õZ¿Ó•nË©zý¿à÷†<x4¿Ý'û»¼rüAGNbll?ïÀs'"ïf?s‡Ig?h!/1gG_?bÖI§®¥-?sµÔ€§ÝŽ?l
JXT/ ?èÿýËÐ×?ÌwØ*ñ<»? Ãn3¢4?ž÷¢Ã¡Æ]?Çÿ·-±Ç–?ÉÝ:½/Ð?î*@×ÿ9?":Q® Q?•Æž.P?"-FOÅ?¢xøEhÃM?Ž!Äp¾Ì2?ë£ËÍ&ž?¶2$c­?ˆ´x2º¿?}Û¸f# ?¿áK	Î9?¯sb²®'?ïäÀ™+¶?_•x­§Í?U;ƒf³[?NŸËÖci©?`¢qèyHe?V¶ñígW?ít¦b¾?º"ؼÌ,?ŽrJOxpý?'>¤Þúª^?°'©''8t?·›vŒ¥ö?ïL"–lµØ?6˜ˆ™Œo?"5~+E?rTŽÚDJÛ?ˆÅ/¬T­?v¿Y=|@ý?î—].¯?ô?¢~Zî?wµø>A?_p!'T?£"ntz:?>i'AGN3FGL J1354.5+3705@RišÀ
F«@RXŸá²7À:|¼A%À;üÔyixj¿±"Jn@
(oxùt@LŸ•Ü÷¿Ü$ÖN*ÛK¿áµ¸r©¿è†ñêR¿ßó(ôy-AGNbll?ï¹¥æâ€F?€Iïß_Å7?ttùÀ^?y.94;³?n;0ÕÐIŒ?lSϲp°5?ïR7HZg?›+JïX1?"V'žÖ¬ä?ŽäÝø‰¸'?‡›R[‹z?'‰',ÆY,?ívMå:‹?žØ5ç? Ç1tš›G?¿òˆn2?§Óð8©î?•j‰2Yž¡?헴rkŠñ?£à¢m'ÙF?¤Ìì[¢+þ?Ÿ¿Èág?¡·ÌyY¡÷?˜B+K_ï?ïïEŒjö³?^ê°àJ•?Mm˜®oÃÕ?PÕÕÙi©ï?R¾ý¼>Ä?RWvό:!?ïÊñ<1£U?~"X¸²¨?lŒü"›ñù?v@›@Ú°ü?hÇ9À¹?lG¶ï1"ý?ï³ä§°?‡LßU7*?Ž'ÎÂis@?¨9oW?(	éd?zA¯8™yæ?ïže6Ì«ü?z/—È‹+?y
—êŠ%r?fÈð½v|a?wÂÌ«°@§?sñš[fP=AGN3FGL J1355.0-1044@ts<`Ÿ@HŽ¥?À	pÀ9@'
´©À;†ºö
³¸?ì³Jð"'@'È"ÙÁ@ûÿë2>¿à\ùՐã	¿åÞcK†¿éGl°ØO¿áñ±Òº;iAGNfsrq?ïûƒ~±.?8ø˜ "ï?8Kæ4á3æ?4zôüZ#?'0T÷6œÔ?!I§*ö³?ï¿ä1z?}•$À¶_?l¹g±Iü?qâ^c…þ?q±3ÐMF?s·+"Îë?ïÿWDî?ˆÐUªQ‹?Šî¹z˜I#?}УŸk?H¸_ë=Ÿ?ìXqæ"?ï¨BŸôU?ƒ‡!߃ž?`Ÿ{ÜËl­?aU²À+[¨?ÇyI?«'?'«
dò?ïý«àK¸C?%ÿ©·£Æ?*dxV		?"òu¾ïDä?»÷ãp7?H^'•–?ï鎑D
?bPcíe
?TVY6S)?Qÿ]!Ôö?XŒÛ²y'Ÿ?XmU°™
?ï‰
çÔSï?z£Dóaý?~3Êæû,?qyo$ŒJ?}FÁ…pí©?oû&íºÍ?ïðNç;/x?[™Â$MuR?Gã'ùÓH¢?<¿Ý$Ü¡ã?Spoꡱ…?XëЉ;AGN3FGL J1356.3-4029@sÀüßï¿@@4¹&Ÿ¦ùÔÀ:+qøjàIÀ;®2Ì&°¿áÆ(Ûìz@Y0‹yp@{P@4M¿èî)jª¿â°´ a'¿çÿ'z9ÏQ?Ô6aË÷åªAGNbcu?ïð
ÿYß<?TWŽeíb?CÙ¯ØJl?BÉ	­€'Ã?Uý)VÝ?Nàó?ï¶ò>²?' Í㟸r?kxDËé"p?m5@4¾j?vʾ'â÷J?}óÁ)?îÿA•»Ws?†²"V,´?‹$XÏÏá?z¤"hßû?'… Û…¶ß?|=uI_ÇÊ?ï£4ÐÎ?'¯­æ+e?,Ž øœ¬?@ƒõ²çü?†À¿þQ6ü?ö¸Àîv?ïúDyN??}R|ÇD?/Ҙ î!?0U—˘?=òéR	`Û?6ŸÙTöJ?ïäŒy è?dA¯4yñì?VÔá'Ԅ?RH'?`iœ,Å%§?]õ•Vž?ï#søuG?t'ʳ¼`?~Mª's?hôûo@`?MÐÏX?h¥~¯Qu?ïñ¡U¼0?U¡Àê¡`?PlƒÌ¬?òšH³0ä?\y¸>?UYj8ZÊßAGN3FGL J1356.6-6428@s^-••Àð[ b 1À7ær/ÈEÀ:µ'v©V?ñ+$®¶j@U$Zþ@|'@Y·V¿äOEAÊòú¿é>'úeƒµ¿èyæ¼É/Å¿ëÇѺ66PSRPSR?ÛØ{—?ÅʈÏÇÓê?Êø²"žÞ?ÂÂ
gWä?×wôÎs•ú?ÆÈ6Êõæ?¡z¨g½©n?¯ó/I/#"?ÙܒQ´\?ÃÒ5Œ©Ç?áúPùË;?Æ7®­|ûS?Ø7<û'Žç?µ²[Òü¡-?ÍhQéè͛?¬ãJKTq"?Ùšz
L?µ}ÁZ‡³?Âaù£Åm?§
påN?ØwvÛÅÛ?µ¿ê
¿.{?ÞXhRWn?´W+"Š>?åèрÚ¾?Ã;õN¡#?Â7gF?ºl¦'W^?Æ% ˜¼Nû?½5Q+8?¶ÿ7ïͱ8?Àؼ­x|F?Úo,mÇ-Ñ?¼<ÑJ=™q?ßÑ•"ûÂ?Ãs/ébëÄ?ã
›ye"?²Ê·(ÜÔ?Ç$	ÎÏ +?©fç?%?̱ˆKœO?­\Qú–l?ÓOÌÔâùh?«^6½½v?Ó¤ˆu"ç[?ª=¨ý٘?Ùª´…>?«èºQë,MIXED3FGL J1357.5+0125@u?€ß×@MæÃ`<€ºÀ:p
TÙÀ;£'wŒ(˜¿ÿ;WýB
'@x_ã@#lYA:¿ézcp½­J¿ß¿üõ‰"y¿çˆ\›Cé¿Ä…âØ|ÙDAGNbll?ïùkDF?FqÚJk¦ã??ßè(5Ù?>#ñP¬—+?7LÀßHÏ(?5›n®#r?ï»JޗòÈ?‡'Ñý¤‹.?li=ˈ«?÷«ê÷Q¨?t%ñË»Å?v⍷7‹?ï$ØÈ¿³?…ódGD'?ˆW¡Ív"?{`5 _?Žr¼8"–Ü?w'Á>[S?ïÇ/‹Ö.î?tçñÈcx?²yn°­2?!m˜þIã?|pAÀñv?tÈ­¢Ÿ?ïý
h.£¾?0vº2ƒ?*€-"sҝ?(0ԝºÍ¢?$©NaÙ;½?`vØçqÆ?ïéŸD9¦ü?cBú÷8£?RŸùÝÒÔ?R!=í–?Z!}ü¡¥þ?Yïüöù+?p=k?qÊQìÕ7?zœÚçвØ?itü¿\Ž?{–í)}´?bñO­L1ç?ïö"{™ö®?K»Å´´>áj¥®íJŠ>ãw¸¶?R´3¹Ãî?K§¶æM%ÉAGN3FGL J1357.6+7643@]ƒ5Á'ì¯@CâÍÀÓgÀ9Gêz\½À<'ÇÅý?òjêD+þá@ŒgH8¨é@ßs¿jc¡¿åq8b®1¿äÍ$oËë¿á Š.öN¿ï ¯?‰AGNfsrq?ï¹°˜\?Y'è=ì?|&Ÿlèn½?~ªNuñ?]*"Hk\ý?^ª;J?ìbøïW?·€]Þł2?³Ïñ~ÎÄ?²®'>F'P?¢0›(døþ?¢ðF$³'?ì嚡ßìÃ?£îGðÕK¿?²Y$ÐÃ7?¡x¨z‹v?™è}†ZÑ?‹Y'"Q0=?í
o"UH?¨ñ[®nÁ=?±öÃo,½á?£Ò‹¯tlü?–×
ó|œ°?–:
ºY‡Ð?ïßÊ
Oº(?mJP|?kÉãÏúÔõ?k+™Ú†Ç£?A°H3£??Ë"$5OÞ?îs"e;)]?¡ úVµÔ? m,³z0í?™Ót]Iþ?µï?‹ñÚj—P?îCÆvÏó¦?˜qde=%?¤]äpY8¾?"}&g
	Ë?–Ѓ¾ûy?€Ff²4ǽ?ï
ÆJ°0?‰.aJj?šé¡öˆ¨ž?'×£Ð2<¨?m쥓K™€?s·±¡gAGN3FGL J1359.0+5544@Z  ô×®@Mr /µÐÀ9Nû'²õ‹À;ô4-n¿ð-âPíƒQ@Ïl®)±@½¢À^ÕM¿æI6¦kuU¿ä
"£`¿ëJ.‹>ô¿æ…=å):AGNfsrq?ïú©ÕY–Ó?G1ðÿ?6D©ó'?87BÏQ?4mGú!Ω?@°rWŦ?ï½5ùiÁm?€jŠ#6;?l—Wk
?qxs›6‰u?s\·¿¶&?v`°1r&?ï'ó9?‰×Rlw¤?Š³lñžR?'<šûòg?'&$ƒ¢I\?'NJiDb?ïÜ	BÒk?s­†;
%?Ck¦÷?å?KÂÞqšãû?o>ÛßñŒ?s6UÎÿÝ?ïüVõ|Â?W­Äý«&?1†sªpqo?L<¹•÷œY?'ƒÁòÀÎ?EX¸PbN¢?ïå¢j½Qô?e‹Í"x–?VÞ¶üÓÔ?T"z×q?]ÜtÅWÃ?^Îà'ô?=˜?jz¡I¤Ù?.ì/FG@?y $òu'?€"£˜Fðl?s0?w2F?ïûýHâê=?FPòB"=?úPkÈår?ûý4¦P?=¶p8ö,—?F
'¶ðAGN3FGL J1359.2+0204@u+é>ê!@N矶êÀ:Û/fÀ;"ãiÇC÷¿Áò–‰KT@
éá·?œÎ@©Ýÿ¥G¿q&ʚ˜Î¿äk8>¤šB¿âÊ˲4^ñ¿ïê…¼AGNfsrq?îN4dX?§Køӛ0
?¥ÒÚ¢¶>d?¦ñ
¿sW?…HfqA?ÎaÞ½´?í¼37˜?®úFi²%v?¥ôT™=ø?¥öüN¯5n?œ•0f?É?žºn°Ÿ¶?éâú³åË ?ª26I˜ê?À·<H@ò ?¥oj?:²Á?®ócžÎ}?–òف/6?é}vY½Op?±¤ØÖG)G?¹D~u€ÿ}?«\Fðð?ºÏι$é?©^´E¿?ï^Z¶¯Ôï?'GÅÔoŠP?»y˜fK‹?xǘÚ?q[±`›…\?kIvn1?ï`[ÊMõ?‹ÅŸÏ<Ó?‡…6ÉS?ƒ€mѧ@Ž?€c×]"±?}ŠìJöQ?ì<kL‰F?¢¾~›ŠŒ?¶=­˜¾£?Ÿ2•w¢®(?Ÿ{àƒæ¹?#eB¡{•?î=â"w§	?"
'¼«™+?šÐr!DC2?‰Ïam&uÀ?s=H磳?ŽˆòäUØäAGN3FGL J1359.9-3746@sÙtàM/@7#Z0FðÀ9iÀJÞJ¤À;s&îR{?è–îÞ3kV@Z?A3@0rÀ;ïÅ¿å7šÆ•P4¿æ˜û;A–ñ¿Ôì·p;Ÿ¿ÞPF¼v/AGNbll?ïß@žÅlJ?g"FÞ]±H?Q¶LŸï2Î?KÎq'¸"H?gä:çÜlƒ?d5ŜS9?îꀏºü?§:g²?Ž:ÏcôÔÐ?ò~?"'†Q~§ð?¢AXo"?îßåÜZ?‹);(CB?ŠßàÜÁdù?{û6? µˆ?–"om}X?'¯ûÞÅ·?ëÊéÙß?¨l¿qi?4HúR?šYìD1>Y?¿ö¤•(Ï5?¥AY²;
Ÿ?ïòzüu†ë?S¼qãڞß?C 	Ò2PÑ?@éB•y?Q:÷{ì?M"Z©iO?ïªå,¨'?‰!OW—p¾?sC¶ãªR…?q¾àÒM?wI½e%I?ƒ'8§"d?ï€øK^UÔ?wgJÛiŸ?|»x1W}?qNà<³?d1îG%?fÞ,"]Bš?î6¦kuU(?'ygõݒB?—ÿ`ðF(Í?†ÖO¨$? •èÒ?g?†a£[VúAGN3FGL J1400.5-1437@tnݿη‰@Fßä׆À9e=?&À;Š²@YŒc?ñáÐd±ÛZ@
ZMÕ ÛØ@d§ê9?«[ž§~¿á3(N±F'¿äÒõÚ~|¿ïÿK3PSRpsr?¦îà6л^?°zø'H;?éôEg›Î0?Æ}Æ¡±ã_?Âs2Sܘi?Äqã+LΪ?Á§3yîÈ9?ǖŒÐCµó?èËOƒ9ʖ?Ìô0|R>š?¶WôèÝ?¼¹\ː•B?×·)nÛ¢J?µ){Ìŏ?ÝÀS©íœ?ºÇ¿z\p?ÅÎmƒ3?°#×>5‡Ü?Á¦ÄIŠQ?¬]y@©U‰?èõ} £IØ?µVˆ>€ù?µqvµ ?¨2Ÿ/GÑ?·ˆà¼ÀP˜?¹7›'a#Ù?æY8ÎR³×?Ê
Ã|R?ÊÖ¬iÕܖ?ÇïîXsb?ÍJÄת?ÐÅf¦þ?æÛÈéï?Ж³	F¤?´Ìþ1œû¼?³—ýû•x}?ãIÝ.Cà*?²`³¥o¡à?Ҋ´<:Ìb?±1ԛ²ª`?»†EœõÍ*?¤³{ZþÏ
?ØåIÛÁ1c?²e…ö¥õ?á¢wùƒ0™?´¹D"Y˜à?®®1ˆZ? bù©ˆMMIXED3FGL J1400.7-5605@sˆ€CR@ïI$À9É÷/væÀ;!€´Ê?ç/þÛgÅ6@èhÜ7xè@ù{ßto>¿ä;v€Çˆ¿èl5†Ži¿ä~ÒJ‡…¿íˆgS\…AGNbcu?ï˚ЦK.?rf³«ý#?l&°´arÁ?j£Öù—?h>~‰Ö"?c/>/Yl?ì¶|XÁO?¼\%ß|k¥?¶ÿR}r¿?Ž¦ð	á×Ö?¶U=O§ï.?ºjùž?íÁdíH ? ûdOÿ?¦xgcÊ&k?"Œ$£éÍ»?¨Ë'K©‰—?—GQ''…È?ì þ¤z$?£‡Øãò³Z?–÷RŒˆÇ·?‰ Ä<LºØ?¹:69éSî?¢nËöÊ?ïß¡ž©V"?ioì4Ä[?fk­úVú4?f*Õ;:N•?Såfúƒ÷?Qm9¡C¶?îßî-«Åý?¢†ÜŸŠ?~¸ÜóŒÝ?}ÏKõÿN?œT5Qê…$?Ÿnŵ C)?î†ìóçL?"ë°™Ž§?šýà§0l@?‰ї¬?">Á³srY?†Ñéõ°#|?î¬]æBÈ?….Ù-?‹™®—vŒv?rª¡©?œ²œþ[˜¶?'Ň
Ž~AGN3FGL J1404.8+6554@[àE€<ÑB@HÇÀgnÀ:"¤?
À<3ÿn	È׿bÓ(iª5m@ªÕ"ð¸9@¿	 g¿¿å•›Jý1ø¿ÝWp3®¿àþówJS$¿åS"ÜôWAGNbll?ïÏsSÅá?z¹DgâŠ?sઘyð?y«õé³Ù?Q–®"Šæ•?Rƒ$Ø?ïske1f?ˆCsÒr™Ÿ?ò!üš;ö?y+YPýi:?€*#? ?'FÑ%?î¬cªc/>?–K§R§³1?žNß%Þ?•[Ô%×a?ˆ¬w¶¨šª?xD®…	üÅ?ïdSn3†¸?…
+u?*'\ï|?rQ'Á"¿?‡k\X4c?€†½¬ò߀?ïòùŒbò?d<ÑÖ³?UÛðŒàšª?c–òÜ5?0ÇúðÓ0?3™8Æ°ß?ï֙žeõí?r@T#×µ?cn¹+eJ'?`?Xé!Ør?e÷¨S'è¥?l˜Æ¾ËlL?ï|ëþÒ?—œ!WjTp?™¿€Í´˜?—Ó@F{–M?u£~Š´v?a¨qƒdö½?ïáJՈª€?aÀoûrH
?`q¯ '?G»È¯x÷?\†ö¯ïN[?\R©—´AGN3FGL J1404.8+0401@uuS@N¤©@NØ_¨DÀ9±ŽXó·À;šAÿŽÁ¿þöFÖ~&w@
'ZÀëÃ?ÿ¶MAQY¿åüc«ÿ€\¿à<2m»oW¿×ć^X¥Þ¿å2'#ÒºoAGNbll?ï G:H ?†'ñ$]?dƒe€…r?cG‡z?'ÍX	—³"?ƒÉ°Wµh?奄Ð_ÔQ?Œ8ÿ/uK?sàð0¯>T?…"jB{ì?w?§Œ(ÉI?{ûÔmœ8?î"ðlF?'8~¨zӞ?Uód­ì?|QÇk	žo? hä!Ö~!?Œ'}Ô=Ÿ?ï<€ÏÚZ?öl"Ý›?Læzêö?VË!¡oaÇ?—ˆÛsh3n?²þA$g²?ïÚõÈcS?¸IãÆßÞ?RŽ­†Ñ4ú?\E<ߪ+)?kã7ºòÔ?y›Y½T—"?ïå4|kz?f`‰Â0ô?Xö4úYŠ!?W7<ڊPU?\¡ÊŽе?\Ù4þ$ÿ?ïe£Š€™e?~Gv2͌Ú?}ÃìN«]^?l¯ŸG¤?‡µ'+Íj*?wOÁtW's?ïÕÄ+­F¹?kÇcK¢=?ԑf]ÒÍ?|צÎk?t¶—Ä;à?k•w]ž—AGN3FGL J1406.0-2508@t9}sÉ@A[Œ@ÃÀ9¹FMÂ*²À;ƒÈ¸kù?…°ýEÂ@"Mië?þI`½¯ù¿ÃMW<¸ÿ!¿â˜šÿR䇿Æ^,h
L׿äB
s¨fAGNbcu?ï¹Q÷³D)?"‰ސä?]b$—ýä?atoÜcp ?{þ{*v«Ã?ƒ‡\¨?ïN Iê[?–"‹"Zd?"AO"å?ˆü핳õª?ˆ@¬3ev?Ä•G!?îaeUø¸—?—Áâ;ˆ'?‹ßËW+àÙ?mÁRþž?¢ñ·ÈÉd?•[òra?íbZȒD?ŸG
GÚô©?€7U.>-?{‹<t\??²ëN?+£˜?ž"tÃU¾?ïë"t;'&?r/§ZEõn?A‹4"'?=çÉë›ÞI?`&¨ùB}|?q²¢9as?ïÄp,Ò'?wâ˜p?jBtL`´S?cÏ*}ª?p¦¯t©Í}?s7'Tâ­?ï$ñ< uI?ŽèEžý?‡;i»*o?…k¦ £?ˆª€ia?†hÎHô?ïFøÖ|4??|¤«	r^[?tGŽ1£‹?`_'°pô}?'ž½O>?yvókåÞÄAGN3FGL J1406.6+1644@É?áAy@QoÄ`Á
À:ž°²ºÒÏÀ;ÅbôÁÞ\¿Þe¼S>&½@ÁÁnSñ?ú[~ Ai?îôÕÄ¿â–û†è¿Ý	º&_˜Ê¿¡ï¢î4¯AGNbll?ïê}­ˆl~?bé'
äÜ?D*á1
?Aƒò¿5?`}Ǹ=Ü?_ˆ¥Ü?ïÁÁ—ÿ)…?|"ZÈ\´?kjL(:o\?o5…kaêU?qj
сå?rÂELޒ?î¹'cœ1¤?Œjyœ?Ž€Æ^Օ¢?I}Õ^'?™š°W疩?"×o$U>?ïSnÁ¥°?'fÀÛ%JÕ?Kå(ÁpÊW?Wf˶)KÄ?"³…qX-?',œ)ç'?ïøcñììÓ?D<ƒ?ú?-âJO*`C?%‰à|y?F÷¦*oW?Añn"·?ïç D1÷ä?h%d,i.?U{|\ož?S¾ý±½?\Cû²/i?bå¨Ú·î…?ï\~«¬–¡?€•¹æm>?r‹òq?vžUC†?‡nOIUA?u5*'öxr?ïâ\ÜØf<?h#ë;µ?2 (›Š{?0禬ÏnÏ?kOû²_?g˜p>ùZ_AGN3FGL J1407.7-4256@s×àßÞøH@1¯3+¦À9½ø¨ó©°À;˜êË»TÕ¿óDçÈüˆ§@ÖðäJ7@Éd~Û¿â}^â'kÄ¿æ0²
»¿Å%Þ®CM¿ìR€‰ŽoÖAGNbcu?îöÆìk¬)?ž÷'»®,Ô?†~@@2?Žöã.Š˜O?•ÞãsÙö¿?˜4(M<xö?ïP¬B"£`?"ÛË<ôÂ?€ñ !6F9?~hö‰j¿•?ŠãO@-£?í³Ù(?ëþßîVy"?¥vÏEÐP?°È"¾–(K?›W
ü?®€÷›´OH?›ã#ºë
?îwC^W+é?Ÿ…òʙ^?c¼
wåÒF?o2Éû¼ò?§P	DÈÃ?ž\	Ù,2Œ?ï_áõRýÔ?®ŽÂoõ?t ,S\"?xÃòg¡Þç?·l¤6þ?®bƒaV®¤?ïÆÐ㡔T?{±g]àš…?f'üÔém?cÔå"S½w?qN¹xµˆ?unxm?í§O¸'›"?Ÿ sáû½c?¥6"(F¯¸?"Ò|$˜Ú? T€O˜?"o r«Â?ï¤JÌa‡?{4֌Q?B¤Þ"¯h?@Ý¿`~˜?…Ã0›óì?zÀŒ&†RóAGN3FGL J1408.8-0751@tÝ ßÞøH@I'æ@;YrÀ8|«ÆÂǐÀ;SÀ'U'z?ïM,6G@u ,°¸@	ä ¦hµ¿âºp‰ ¿ç-þQ:kr¿åÞ°Á¿äTjõ䕎AGNfsrq?ïû"drµ?9k>?ôÉ?2C\™B?+$r?±d?4©Qø@?0ÙÖ8nûó?Åâ?ô ???{Ѭ)oE?"®w7Ÿž?Ÿè¡4³?…H'd"?ï?],DÆG?ƒ%"êÔó?ƒAÉjö?w!/bá§?Œ‹sÒdÛ/?zHl!†£v?î>ömZ ˆ?›¢T7gã?Ž{ÆYr
?…Ÿ1ñÛI?£É[H
%|?™ªhÎêl?ïýíÒ½÷?$¨}–0·.?#yk!þ§?µ9û{§?RÔ.Žè&?
l2͝Ð?ïÔf'?qªÛ?cý§NMÁÛ?^
¸ÌTùÍ?gùò@—ÿI?jò³2¿<c?ï"`Cã?q[Zæ Ég?x˜`¼áè?aÀËöÜÀ^?}b†Ê¨é?h†ììóv?ï€Ëú¿Ï8?€w©ód?}À¶€,#?g>ŷւÅ?€ì÷|³5Ë?|bl7AGN3FGL J1409.7-6132@sÝàP7P¿±9RŸô¢`À7|[TŠœÀ9±]ïŸ_¬?ð™!ï¾ê6@‡Ý­oº@ïÀ—µ>¿âÜÌG€&¿á£Ó<Ÿæ¿å°å"«s¿ë†}]#PSRPSR?PAMï
?MqVZ];?Î!P=Ù?ÈÊP%‡N?èo›—ƒ.?ÈÐú°&ñ?]@4‰°©'?u0Goz6?×
ÐNÈ¡*?ÂȤQ·
v?äk÷½ïÂÏ?Âø8哆õ?°01|øï®?š¼P"¹/º?ÖW™"À
;?¶˜pèøó?âÎ->Éá­?·µ:ÛòOU?"ÚüòL?"Ä~ØIÄ?ÇÐm՛}?¶Z1À:™ä?és~æž?ºO©S©}ñ?8ã2fÀ­?=mcÙX'?Êyņåë_?É{œ؋?é^r7ïŸN?É&+I.?oˆšZïË?ƒä<ê'å¸?Ùpu³áC|?À"Ã×ä5¨?ã(<‹»Nd?À¨^£¤_p?·4p¬¥
?¢îÚr€?Õ&Ó,Ò	ç?´Ò›×ð?↻eé‹?µ¹À¦$¢?•ÁG$Û`? >*XÕ?s?ÃPfñH$?°8ºêO©?ê}ïí8R,?¶úU*B¸{OTHER3FGL J1410.4+2821@DÅk 	ŠÃ@R4¿û-2À:IÚÓöÀ;滵MTG¿÷ÖÞñ'@
‰%Bû?ÿ˜ nJ¿ì¦½!Å2á?±šnHæ\¿ä'ø<‰•¿ÊŠûô$!AGNbll?ïð†ÓnQ—?S-Ógc™?FKzÔÀ?EÛùwà5?Sª3 æqé?JØÇ-÷.™?﹤!:•Ü?†œŒ"ا'?o¶:•L_Ù?Õ –íÿ?sRҏ'G?vÛieþÆ?îî¸d,qÅ?"dÞ³H|$?‰JäƒM?v;#®+Î?•›Nx´?|L6Íç?ïÁ/-Ñ/Ä?wü*C±–Í?Jº†A"#?Q V_z¿Z?|_í?v¿¯.±?ïø¯ìÂ5š?BBÆÙW;?4ÑV]j£?3ѕBI·?B×Âì';?8ƒ!¾æ"Û?ïæÀ¼R ?eF?­$è?VËße:Ò?TÃÀ3·<˜?[²¨­·t}?]ÌƐÊGt?ïp˜àGd)?v.ڄ€Æ?ôy[ƒ?l‹Pƒ´3?"Í´8äF?k¶;ʉ6,?ïönG†Q?MÉ×|>vÞ?ÄóµSzr?ø)IVä?QÄÓ߆§ë?M>…™¤"úAGN3FGL J1412.0+5249@X‡, zû@N  	ö#À: H{™ÔRÀ;ûã±ëŸ÷?åϐé>?@éþ³ú™@L_ª	©¿ædÈÉ\Ï¿ëKúo¿ä¸%3ÒP«?Ɓ¡?Ö.ËAGNbcu?ïúÄ!, r?@o¼yÊ®6?4˜Z³zé?4hæ20Ý?5Þ^Ï8´y?3–|q[ú?ïªÜ«ÒB?Â¶Aœ·Ä?sé³Ü³Æ?†éŒïm?v§ö³ãã8?wµ#Zœ‡v?|ô·?‹kË(}²?ŒS)@í»B?|îóJæ/?š›½'¤W?"í&C Ý?ï†ÆN"žÄ?Œ"â7§"?h®…è£?¿â_,t¡?ˆGå5¾À?…žؼ??ïü¹‹@TH?69mNPA?'38S½ô?(™YeÃí?-4[Ùìi?,Ó(ÀcŒ'?ïàªåá&?q%fçù¢'?\³›ø•dÃ?cNç
?`ûL¿YÈL?b"ìÁL¥?ïr
QÞUG?|P Éî[?z(ߥsÛ?d´86[à?†h;¾øà?yP»k:àu?ïéíoÃÚ?sCNVͳ§?T<DÛýnb?l}–&âÁ?WèÝýþ?c±f‡üfAGN3FGL J1413.2-6518@su`4óþÀ8Ô ~$ÉÀ9 ½zIrÀ:ï-؀_6?äI4Þ%‡@Ai×µ@j±€k^¿Ô®<ƒ¾æÛ¿èå*¡¿,ü¿å«ˆ†½Ò¿ã5ގ¿ùAGNsey?ä1	?Ðú'm‹ì?·ë,•QŽÓ?¸@"ÜFˆ?ÑÿÀ>@z?Ìù2è¾?à:ȵ)Ü·?Ój1´OtÕ?´·s<Ù<V?±,•ÿ?Ú\'Æ't\?Ñ[†ºÿP?æ%Ž4Øò?µñ盿•€?¸a¼pç§L?¢K$[íÌ?Ë:㍥çÓ?² 1¨ŠR?ãd?Ùùtå?³RyŤ?¦PŒ®æE?Yµ¹[	?ÖmnËî3-?²[JÉ?éûúÞò­÷?ÒÞy…ÛK? —UéãÖK?°~A£÷1?Ãê?	¼R'?ÐkZ¸?èÄý+þû7?Îx&­=æ@?¥ö®Ýˆï?©—ñßÍ?Çn_—rÖj?Éß–·Š?ìÀêoЦ?£RI¹\'?¤,~VÄ?"wȕXã?¯Äà%afâ?›‡òbÓs?ê)BV?£)˜£<á? òì n\?ˆ2"®€å?òž¶—‰Ó?¡2ÊY_TÀAGN3FGL J1413.4-6205@s…ÿ@O¿çP®-ø6À6WQ'©"À9íi›¥"@+Hˆ"ôF@»¦9:3X?ÿôÀŒÉ¿Îà%¡¥,¿à;5Ý\'¿ãÇÇ)þ3Ö¿ìßØ/wåPSRPSR?"u­Ð¢[?N#Óñ:?ïOŠº·)*?–ë–˜[¡©?•é½J-2¯?–Úÿä°9?±ïº–0?AJvÆö?ë#	ËÁñ
?µ¥ß.@‰?ÃqB"߁–?µsÐMþ?{嶒 ™z?xB0²À~*?ëÈҞÀAq?«ð¾DxôÁ?¿ûža2(?«}m±6ØÕ?P^Ú\mÄ?PÐÿ|Ï?ì20¾ê?ª\HUYMÏ?¾-~úÔ?ª7`ç¼áI?nQƒã?Ñ#ÀE?ïj
¥J}?"ùK?'°¶{-œ?"k)?$v•f%1¯?AŸQÖ/k?ê›?WóuÈ?±C'GˆW?ōäúÀûÞ?±C‡ÒuÜ?wš›5¦¯?~éMñ®c??ì-brL3ñ?¨Þ†ªô?½Jôšò	?¨CíÖâÄ>?TºÂ<¨O?N­*ØCӚ?ìN
F²?¡v™ÙŽ?½8¬žúÑ?¡x.¡êP4PSR3FGL J1415.0-1001@tæÿëJ@G׌àM³À:1¨oö2!À;¢\Gÿs?ñÇQ'ºÚ@I O–@I@ô\ mf¿æV*ۏ¢¿ê&J¿éÔ)¯É(¿á»z	äãÍAGNfsrq?ïnKšˆ,	?'Ž¹6…Á?|ã2°O•I?'¯¢
?…û€‹£?‡û3ãR?î¿õ7hæ¸?®ƒ>Íëç·?–
031WQ?¥ŠËÅl¯v?'ô(ã!m¦? ›ýåÞ£?ë•2Ky™?¨Òäí>­?³ÿ¶ˆV•?¡~"Bˆ3í?®­ÛÜ9pG?šöìü…0³?è?Øv_i?½Ô§ë¥?Á¶fgþõ?¼·$«Tç?º"p$€<ü?ªgç%*ÁQ?ï¬ãSÞ	Ç?†·[ß?dF?tŽ¬¥jÖ3?wGæ3?tÿ©i€'2?z½°ôÚÕõ?嗀µµ®ù?‰`EÍÛ?xˆéþHá>?…o؍ǿ¢?s0;A¬–?}°ï³kü¢?í•ñ'Jê?€ëñ¤I?§…¹¼Ž?"cRåÊ"?ŸÄA¡±?Ž'þ•?ìð*«þm?§f¸Nn+?³
ñò­#?¥Úy@…A£?•Æ³»ÖEÍ?†˜T^ÌËAGN3FGL J1415.2+4832@VÖÿÚ@S@Om€6EÀ:9¤$èîÀ<™RKý/?ÒõË'tÚ@çŠizî@Y¿Xš÷¿ìX¬Œîîé¿ã€—.5¿Þø¢æ@ޏ¿é«ÊCZ°AGNbll?ïî.Âò>²?a.^ª]˳?\Ziõ¾eÝ?_Ÿlã÷?= A›¦f`?<)ė½Ð??溜é?˜˜Bà[?/×Ñ3?Z53F1?‹¶Žô"^º?‡ˆAyêI?î|*3ûD?"ŠOhŒË?–­\ÏKȤ?ŠלKµ?™Í\Éídì?‡ß""?îFý;:ÏÆ?œ Zó©uÿ?ŸÿÓm!à?''m´Öe?— …-<Sa?Œ¿Ö*L?ïùÂú™—I?Av´g-?B5#¶‰?>‰¤a`ä?+Ä·a2?#>¬@Õ_¸?ï¹é×ZÖv?yý²^ëª?r`]3`?o±i8
¯ó?pª·¼Ms?puq§|?ïh(-¤0ª?€™#†N°?ƒZÍBËÒ?x†uÒÎo?'›'Bù÷–?s[k¶‡f?ï™N±¥U?v2˜¥ž¾?'§È]ˆ»‹?kFV!†ú¼?l-§ôÌ?iUý8SœHAGN3FGL J1416.0+1325@) -@P}MÿÒ³—À9·Ät8·À;ÃûkEÉ8¿ä‹×<oûn@°1вŠ@èS`¥1R¿å4—Ö á¿ã2δX¿ãp	Ö©¬¿çˆ\¢d»¹AGNbcu?ïùåÂ2?AAPñ|?0ó{nÕ¢?1òÆk!YN??Þs"rÍ?9?î;'f]?ï±Ú 'Æ?'ª•SZŽ?qÆÉqÞG©?u«"äk3‡?uKægcu ?wÊùã,Fò?ïaiS×?{=0¥¡Ó?|YH?g–"àv÷?‰ž'àn"|?sŸ4ÛªC?ï"&# ?€í<½KS©?^t™žð)?Uü&%‰t"?‡kcI}+ã?íµîCñ?ïýù5ò'i?%FÜÁN'A?¼¼"©?äe¼^¡ž?#DS¸g?dÚï&^?ïå'Qñ?d­ûTåT—?Wã" {!•?ThoØŽŽ?\ú;"‹K•?[µ°l¢?ïºm¬"T¶?gáF{?^‹?mN"w'kz?c27ÚÎÌ?t!ç–/·h?WmÒnáÚÝ?ïíZ§I
C?ZÊëF?6¿ô];èÚ?1}Š??_š´ˆœØ?Xɝ¯A7AGN3FGL J1416.1-2417@th€àe0@AT"¤%À9éé8=^/À;ŠçɨU?ÁJdI£@
ÕQßñ—²?ý¤ã!"ž¿æ´ëQ+Ÿ¿Ôàña׋m¿Ñ¾Ò¬=hʿܱѪAGNbll?ïäÄßmŽ?f=̝᪐?Kvqَg?DªMêE?e.]µ¹?cH"˜Fƒ€?ï"Ù1ù¼?Š^'I¨œj?y*™Tyþ?sŒó…« Œ?'ž5î£?†iYýû­†?îÆÈé_Ìç?ŽXAmY?Šh°ºêÄ|?zVqM¸$?™òŠv'ï?‡jÔ$Óö—?î‡)F—¶b?"¹,¨«ú?v¿Mi´‰h?rJԙ-»¶?¤µëGÏ1?'§ò¼V¹?ïó®Í?\C^¬
Bû?:v¢Ž×¿?@5Ë(ú8?R`‹Îªp?Vª‰ên°!?ïו*ý=?p­µ$F4?a½)I°J?X:ìÿ¶ó¶?f­«Çàÿ?kßâo¤Ë?ïqàé ~K?~êð´ò?}Õº¯Xe¤?rR"I?"œè="V?uVTõùŠ|?PŒ_t?t'Ø#'?nÆË®¥&Ž?]:ù¾+ü?ƒ¬øèOÝR?q2ãǃAGN3FGL J1417.8+2540@@Âõ`iÍ#@Q§š_ý–™À:@җçè²À;äOªb>¹¿Â>­"@$f@wBIP«ê@O=f'@¿ä=ÆҌÕ;¿ç#HÖ¢Rj¿ÐèyïÊŒ¿Ør%åumÉAGNbll?ïõòÞ·äf?L'=áVy±?!*J÷Ñré?y/‡Ôb?Qôùkƒ2,?JÞ$¼îRI?ï°KEè[b?‡Òª#­ï?r£.BÞvî?'Òœi]‰Ä?u7.Ñ2çÑ?uQŠÖˆ?ï<:k5Ù?€Å*q¸?€²—·­.	?o%gB¯R?fÁÐú?w‹ô¦î´?ï€}'%VÒ?'eQǪšd?WÀÄ{¦†À?`ÿø¯¼ä'?Œèƒ.ØÑ?€í'
É?ïûÁWÚ»?5+ò/õ?žl֐C?ŒÜS³ñ?<P"ó?3>èßW1ù?ï㮛çÛ$?i9…6¨	&?ZÎú醒?`BkÝæ$?]ÓÌÞO"?ZußR"ô	?ïŸúò$D?m–˰ƒ?r"FQÖ?V%'¾‡Iì?}~n±=Ä?fØbNI$9?ïé*(Ñ
,?ZȽÐ%?FìbÌÌ?9S펞>?a¾ºÀѱ?W_šœgAGN3FGL J1418.4-0233@uYO d#–@JÓ`IôÀ8C¾vÈ´9À:§dd-§?óșSù|X@¿¿
œ?òº0»3È/¿«1œÜ]þ¿ÓٖG2L6¿É|µ»ÁÀ¿Úñ3ÉÜžAGNbll?ïU!rœ?¢3e…5¢?j J©x?x<Àb¡®é?'Óéôc? ]·ÿÖÒo?ï|"$²s?êÍW¥ó?€#ô	}[c?…É/Ä?€·Æèáó?‡Šå2›+?éDV£¯¤?²#è«dB+?µä bŒlS?¤âh0ê#b?¿ù*fz'?¬±#)3?è<‰ü¡.l?¸®»@'ª-?—€©ÙcÑ9?—fmóq?ÌÂÑ©Þê?¸D\Vf?Ú?ïœVWþ?«°‰–x?e9ºå-f¢?vÔ´­3?ƒ›ûwá?©…ÊÒ2ž?ïÇOá1?ߗR%?k†ä&'æ?sE•½—QÍ?m*,†"?sj‰/FÈ?ê-C¶ýÇZ?°Ð_oÐh%?µšÐ¾Xr?§I"Z°è¥?¸øGu›ž¾?¦ìÂNƒ@ž?ëºÁYÒm?¤'&gF*õ?¢Jw¡ð?ÓÈx¸?¹¹p,ž?¡Þ­kzÐÀAGN3FGL J1418.5+3543@O˜XóÖ&@Qe`&±EÀ8Ml+¢E:À;<º¾­OY?ê6©a…"Œ@<cϳ1@w§€)Ú¿á7ñÓdÞ¿áQ<{0wí¿Ý&¤ãu¿åh^©AGNBCU?ïþ
èSš?!|FYûþÏ?!µ§QîKy?"Ú4¡ŸŽ?Òì‰_Žñ?m%È?@?ïÅ.xÁæG?‡$ŒÂ?l"¯{`z?'¢—gÊX?n<×Þ6P?t7SÐuòu?ïv'´U»&?€1å³?~{õBÜy`?x)xYåòá?ƒXWéK¸?p ùT×&$?ïù%ý"iu?Vn§üQ€k?²-§ë¶?#I]Ҍǎ?Jç'Š«?V9oh"?ïþ™¤	Õ?$ú-0'Åß?…Ùîî®
?#Žl–Þž?E¥"
9?[ˆ"?ïê²Ć?d2,üL?SvO•§
2?Sl"xßê~?XhKáx{?YIÎYWÀ?ï©g{þíË?u/px;ž?tç@¾¦ŒN?rä±Ã?veB'z*?a5¸®gø?ïÿš‡?'ô¡"P>ðÇ'U
{>üØ_—®·?ÎÕ?&EVò6AGN3FGL J1418.6-6058@s•òä?À« ƒ¥‰À5ä°S'ˆÀ9m˜‰Ï@>Î 3ý@¶ÓŠ"Õ?þäE,ã¿ÉrÔÚs«¿â"èCî
Ý¿æl@·øvÁ¿ì·ã8ÉöPSRPSR?<à·g¤?<¸j+ï?æàbáv§ý?йÚåœÚõ?Ò8yŔ?иMì>y…?=ÿL8Ǜö?aCº!?èßHƒó·?·ý•Î{&&?Ìsà!"M¥?¸''¿Ÿƒ?~ͨôdC1?}'´:}×?çY2[?¹ß{:³Û?ÑZ)"ŸM?¹"ŒË½Ê?[í¨QOÎS?_pw%ï/{?àR4Í8?ÀÙAS¡+£?ß?¨½à!?ÀîZ"@Üa?4x3T­Œ¯?6ô?´I=ú?éµÏžýö?Ì5Áêö?˂ì¦S]Â?ÌŽ<ªf'?PJ-ŽId?f%Á&n³K?ê$ìø«Ô?±ãëÞ¾o?ÇK·ÂJ`?±âçrƒ"?}ûüRZò"?€Òƒj5,w?çW;êM!'?µqR	A…!?Ð٘:|†A?µeh5Ç­Á?SO'<çW4?UŠ…s'°?â¯É"Ü?ºíŦýl?ÛëPìÄ¡?»~ž€PSR3FGL J1418.9+7731@]@ù?ò^W@CK. &{•À9óË!ÑáàÀ;àƏ›éÖ?êªÑI´)@'œH 'Â?þ€*Ÿæºµ¿èr|Ë$#¿ÖH
y©ÿ¿Û¼^ØÏ¿à¼#p·<AGNbcu?ïó
wŽh?W
7¢¸äÿ?PVvrï†Ì?R4+®jE?C)5–x"Â?@ýFwž?ïU<Sݬ?"üæ'hf?"tØ­?‡nïÄ@Ç?†"wÜLs?8Þ\±?ï9JâÁ3?Žn®²<?Ž(µÔ,?Š.‡Ù¦ð‡?ƒ"Vâ+ƒ?sêOŽ‡¥?îªî¾í™ª?–Tß:Úê?'¼Ø(™¨è?‹5Y"ÿÏF?˜åOòÓéï?Žÿ‰É©?ïúçL³k?A@'‰1Š??#B)kù?<Aބø¨>?0uƒîP؀?%°/$wžV?ïÉu7ö¢š?tL-‰?i4sHýÂß?aºÆÑ:c·?mVTžŠö?qtÉÌÙ_?ïœ$¾¡;?|\Ì㶱Í?}§è8!}S?yPCÀV"?tFzkÝ?c"n*¾?ï"‡%8?vŒ+¬]ø?'F©üU?naė™ñ?qohcXÏV?iRSªÀAGN3FGL J1419.1-5156@sÆ>KZ@!?" ÔÇÀ99rãLkÀ;¦-?Û¸çV96@
úßڛ—@LÀL
ð¿æKQýE2¿éH<Mtc:¿íù•©
³?¹Éi–AGNbcu?êgÒnB²?ÂMóµ™Õ?°§`ˆ6?°ÏPîV ¦?¼©Å1‰ 6?¾ÆF5nvÖ?íaeI/¨?¿þró‰ò?"«×äÌք?§Ýá~&û?°	ß¾M?¹7Ÿ&~øa?èmé7?±æˆø.ê?²gôu9;V? —ÕJ$z?Ų!-É?­Ÿ—Ar§?çämÌÐí]?ÀÒð<éjg?›'‡wE@?¨Ùy9š?Ͷ}¼)£?ÀA£µ¢â?îj'̔?µõ-·Dæ"?•ÔçKÉÅ?¢+3ޟu5?¤žä1Bm8?¯&1é˜EÃ?ï8.{y¯*?¥&'ŒìõÓ?z™Š'#A?‰Ê]ú?'SΩT‡?žroȵœø?íöÓû?f™qh"‹?¡o…ê}F?¸CØæÄA?®"ìÀ	?—)¶Î+ô/?í¿ŒNq@ú?¡…PÐ;¼ü?€éS4í2?\\@U')?° _ÿ–?¡P3=&ùAGN3FGL J1419.5-0836@u
–Óõ¶@H0%ŸÌ¹'À9ñ|¯~À;~i%]‡›?ópò~$@BwsÔä@)ñŸj¿ÕÐÉöG‰E¿äZÚŒ_¨¿ç4L—wV¿çd^¾/AGNbcu?ïñülÖº?Yˆ6¸<U?TəÁ.¦?Wí²Ð7i?<ö3'áÇÜ?6«á¹ƒx?ïŸihék?†~¾JH»•?v|‰);8?u?v®w=?yÎÂg†€?'  ¢?îhAo¶ò?™ڒí‰Ú?žV{ʗ6•?""¶LqŒy?"¡V5ó€6?‰:îO€6?îþ—…uÔ?" "µR+?‡2ÍÏڇñ?€¥tx2Ñ?"¤†/û'?'-Šƒ¥\3?ïú1,äv?Aÿ§Yd?A›í¾È¨??ãÐÔrö?&(¨Ê‡? Ǐï--?ïÛo\%½ ?m½]û?aIû¦pï?Y›±ïQ?cY¿é?gCº	¾?ï]ò›à¾?ŒÊ!kÛQ?'"÷ˆ,?‡>Ë@%w?…¾"E‰Üi?{t¼zvg?ï·£¸Vs)?u	l*?­Œ?u¯˜÷Äg?gÀ†'7?lýšg?l¦.QðÁAGN3FGL J1419.5+0449@uâê@M®Q¿æ4}À:•ža÷À;¾Љð?Ïêé˜_ˆ@
&Î 4?ümá]?ìÅt¾:Z;¿ÔÂ
@ºt¿ä;ÝâÚç?ÔÁš	.ÏAGNbll?ïñ§Róþ?Oø*Œ|c?> ~±YÞ.?7#³ì¼k/?U	<«G{?J]Ý ÎÔ±?ïÀ­|¥m?'ZĶm?köà™Í¹ä?o-ws€o?q­ÑUcÜä?vÏÁC?îÚ'¬tñ!?‹Œ6:ÁËQ?«'Ý?p?}Óâzéí"?•åAa(?'«qúÃ{ý?ï1iÈ#Mk?•šU;ÔÂ?j:"Àdˆ?{Än†|Л?–‹t',&?"[¨ì?ïù"š|?Nã¨oHâ£?-}X:ÚÈ?)gÕítf?DB\
C¤?L«¿¼ðÊÙ?ïä%öø¬?hgaÂ'+?Y¡î²ȉ?Wè½IJ?^âáA?a²¸K êÐ?ïlÐÏL<?w7­ ÷ƒÈ?€Þ5^íZf?o/£ɝT?ƒí–ÀO&¶?j~æzöÓË?ï݂ÊþŸ
?qõ·dIBw?IM®×<ì?T?0<ÁÐè?l8áv¾ªv?o–Ð[ヰAGN3FGL J1419.8+3819@QlT_Ó¥.@Q³çüÔÀ9˜ov°`…À;ãžs.?ÚÊ4Sf%ñ@
qœ÷GÍ@êÃyíؿݺÈÆáY¿æHÓ¿–i ¿èÀ…tQ¿ãäVpœlªAGNfsrq?íc2&ù(?±ý;îW[è?¥LBÖ#?§DR‹ÛCr?¤°'†9e]?¤nF®µì~?íÔì‹%"ì?·F|&œ@?¦'ðŠÇ7Å?²àµäˆ=A?™‡xÀí? qØÂEם?ëõ`V›²?§n+=Ü´•?¥ð/ô׆N?•ðçàn?µ[Ý—-G?¡"^}q—]?è??×ö?¸¾2O9wf?Å?>=l5ø?¶†k;¹q?³‰ƒÔ.˜?­>3ü¸¡?ï}®ý‡?"qÄë?
%Æ Ö?†™‡·*4m?æÝâ?‡—»Ì^Ý?ïqŒùçÑÐ?›{©µÊB?…}–Á,?–¯7K×Õü?|>V'{Ú?'ÓlH›6?î³½½÷X"?…õ²u6?Ø¾(
H?€èËá¸gË?˜°4‰Ì&r?‡"®O?î^'	¦"K?–‰ßÚtô?¢m%=Ė?‹i–ë–ò?ŽÁ©ˆCÌ?Œ‰ô%¥WÈAGN3FGL J1419.9+5425@X"'`4P@M"ßµ§íÀ9*X R…ßÀ;Õ»¢ç¿À¹u³q˜/@©¤aÒ#@u¼ '+"¿ä%bf_¿å -êÉâã¿áC×ͪ¿äÉâb=ëQAGNbll?ïúÝ8ô?@¶hÈj·?%èÔ™¼ã?%‹'‡Hœ?>#ûµ¾&?<¬v0‰Ä?ï«q'µ{¢?‡Ç£¢nðÈ?r¹)qÏw?´nè±%ó?wŽB¨T?yá›OJÊ?ïP¢óh­?ƒ¶d¯BÕ?|Åön"¶"?pÓOf{ON?tG÷ü«?€5'vŒ?ï™øà¸"W?ƒ½Ybû†?`B¶•G4P?W—MDo†L?…q1u&?'¼†P¸…?ïü]ҁÜ?o|?@Z¬«?oܘh´?$¶ÇÄ+q?6ûû÷¶Ú«?omÁM4Š¥?ïáÉ.õj?h%ö—Ë?[•Ïôk?ž?VXµ{/÷Ä?`l
Fv?aJÚV¾¡¾?﯁®š?vnЃø×?pc¬kdN?mD'*Fª?wÛ|hwä?pæ½Âû^!?ïðYòðð?]øpnÆêÝ?=\¡´wÄ?/q#¼L?X¢•›z?\ì•ã~cAGN3FGL J1420.0-6048@s˜jŽ:Á?Ìb'KÀ6Œd¤ÅFÇÀ9-#'Õ?öèË°íô@& ß²C@õž_§'¿äø²Ñ‡¿á—~ôt(¿åV+8p'¿ê[õ¡âéPSRPSR?dm‡I5U.?fæ@‡¦?ÐZ8õXÌ?ËRéd«è?çàå[ö=?ËeãÌ:"2?xϸÒ¿f?ŠOÝ?ÐÚß·$?ÁŸ3jU??ça[‹ÆÀ?Áßäµ)u£?¬©j«œ/ß?š%`°Æ'1?ց®4?º»-ÃÃË?ã+(ÏEç°?¹ØgRÓB?^6.IÆF?•Jheuê?¶š VbN?©Ý¡4œ?쩺M£ô?°Æ™/{§?`ŠŽ†7‰|?`ª	H¿±?Ðu¿}aˆ?Ï=.ƒ9õ‰?çà:'»²?ÏTokÑ<ý?ˆÆT_>.?•aœ"y8?Ù#Ó/?ÁþiÛnƒÊ?ã
ÿý¦´_?¬€Åû?¶Ý¿·89?£ƒÍ
§|E?Ò¸zRßÿb?´x2
:Èu?ãÈ
ßhA?µ&cSÞ«?Œ™&°'?›N¡9%Y?¶Ÿ"QÓ~º?¥B;¦Ù¤ö?침Ú̌-?¯ðöÝùb0OTHER3FGL J1421.0-1122@tõEߨq¤@Fäq_¾¬yÀ:ï!‹kÀ;¨ñ՚Ѩ?â¥hF‡Æ*@*¦ò—@ƒ{À?˝?ïðHöF¡X¿àKz'°§†¿Ü"ŒM¿é—ðJ'"ÞAGNbcu?ïߌ²Læ/?r´V~ÿÊ?iÌã¬çç?p¿x
[®<?J™ª!1t?Iãûðâ·?ï
šˆ_"? _ Éj•ì?‹¼&ìÒð?‰€Â-­t?n›|
eÆ?šý¢M_hÍ?î?<)}?žç¼ùVSÛ?¡gD³?˜o°5>/£?•NâzÙÆø?†q)Öµ?ì謤cL?§(†;U=?£TŽµ€y?–´ÀìÀ?®)Ö}¥3?¢®Tˆ4ÅÄ?ï÷0ý4.í?PH¸¬?I'nÍ?Nsæs^Œ?2˜îSÁŸÁ?1`~i÷ü?ï±ÜCëÅ¿?€¨ÒpGŠ1?tJߓ8y?qðš—ô?rÆþ'ïë?xx%P?ïáW?"~§µBî?'L$¿ø?Žþ;ëÏ­Ž?…àИfò0?"¬û8TŒ?ïU—žÃ?‰ĄŸy'?0	e·óT?zN×%?‹z´ô`\?ƒ§×–õiAGN3FGL J1422.4+3227@JÅ`Iô@QeæÀ:s¬ ›%À;ÿÀƒé.,¿Ù8Uj'Ï@­¼Åd#@zIŸÜ(à¿ê,‹5¦ú¿áØ:å6ُ¿äoÙ1^¿ïý¤µÎÐÕAGNfsrq?ïõ{l²Ü?ˆ±bà‹JÀ?‰ÛΫá³?ˆ,…uôn"?Nm(sŽm?Pô@8—[?îõ¦·S,½?še"=ñ
…?'ÉÛ?'cû‰{?|šîJ¤?óèjÇ{?ìÉFyYÄ?¡'À'(É)?¯ ¬ÍòÊ_?˜úÖ_o?£Êñ¦,b?"Myw¾'?î…Át? Û
 \¾?¢Ú±lî©?šXœ¼J?˜9åû2(?Ž§&šÕv?ïÅQî+¹?x§>l¨?zËÎ"†X?wž`éÿ×t?DY×Í;p?@áóM
…r?ï¿òÑ:½
?ukâû°	?qÚëH5í?jüÙeO¥±?mÙxÌVo¢?h_âÉ>?îZ8š?"­¢ÔŃq?¡"@þ?P?XªºHþ±?'°j·=?²À»SI?ï±H39W(?u"ã"?uõ³7$w?k±¡J*'?qf36 gt?n
7Z9#dAGN3FGL J1422.4-6137@s˜^`=Wy¿ä¶ŸÇ±À7¿—02ͳÀ:c""aSØ@ðfôUÒÅ@BŒ:áRk?ñ¦õºgš?ïùÎدs?¸žàLÓºŸ¿Ûæøݽ¿ëk$GSšPSRPSR?m¶|ì	?u©T¿éÈ?ìʔ1êwœ?¹Öâ#åÒ?¸¾p»m¿?¹]š9‰D?K˜÷ý	ýñ?…Yπæ'F?å†úb²&Ù?Æbá±,«?Ôä>¾°o?ÆeZúÄÏ?›+2Z[›P?"*ÿgf²
?åá¾õŒ?·*LqØv?҉Ъ83‰?¶xÀRL?ŒçIåL+š?†/&«‡Ð?éhrBÈT?º7Yˆ‡x…?ȏÂY›´?¹aGGe?oušxŸ?w«Ñ#Ñoå?ìt	W .?Á•fóÄ?»cä±2?ÀÜ¿Àí	?P¡y·Ñèë?mdãϳµ?çÁ*‹Us?¾ô'¼~î??Ðm	oâ³`?¾÷cu™>?¨ßõi;?œŒ×Ù	5?åò2,Mþ?µ¿£	(Œ?Ñ‹09?´éÛ(øà?'«U<0?ˆÂI/+¹-?êN
O[?±µTTÜú?'n]2lS?°›<CînPSR3FGL J1422.8-7828@s9(€QÉ÷À0p‡ÀSAÆÀ:VD& }¹À;µü‹×97?ï@"§;@"Õxíҁ@\t_£S­?Í$Ø5¥m&¿ÙÆñ§³Ê¿à\2ce¼¿è)'KãòóAGNfsrq?ïàRį-;?if·0?b¢Lրé?a[ׇ´ìf?ZÞ³±ø%?Y@5¼-Ïè?îÖÀ3?±;.³ªc'?JÎG…¬{?'8(:†º?¦],؅z™?­ŸÌÙ8]?î{ÙZ­S=?–­Dðj£Ç?˜Í×eŒ^¹?Ž®'}ïÛJ?—¶ýIð£'?‡ýq#f‰?ìæk#œ?¦GwLƒS?¢µÜ›KöN?–@ëÃã
9?®éœ·íRå? ÊÅ«XNo?ïôÔñ¼ùÏ?V¿YŸ`?FMôL¿š?D–™Róð|?F^C³Û?R&P¶û¤?ï_v¡
ì?•€ÊKÛN/?zowí,Ä?w…íÃS?‹&\W'.?'>+zPU?ïF³]þ?†–l'@lÊ?‰Jq5<ò?G0«?…	8‰¯"?w)_¶nq?îË
sAQj?ˆMWv´gP?˜¡Š7¿?~2°›"¦{?‹ú $b?~úÀÞQŽyAGN3FGL J1422.8+5801@Ys´á¼©@K˜Z?çvœÀ:‡ëÚ¯
ŸÀ<!µ±þm?鵡,éu®@
V;Í5¨X@$û_\[ö¿ì¾§:õ|ø¿ì^êв¤F?â/ãu/×ß¿Õg¥<AGNbll?ïîÈP¢k?eEW]îø?9»~ø¶˜á?AÉ(¯Y?\ìg"?c°Ö@L?ï¤Áº[?‰Gß³Fxf?wd_	¬¥[?'H!ã҆?v'À !?yYÞ@Y5Í?îÍ
oùÝ?Œ=â†ø'?ˆ6±¥¦ƒ'?I[i	eN?šCY6¡(Ž?…ïc oi?ï}#þH+#?•Bø^\<þ?dX<R¦Ëó?€0ʶd°û?‹ ñNLÄH?"ŽWU®0 ?ïøöñZî?Ey<ãö??"¬¹Ópë°?/fúÿÈÊ?Gyɨ¦5?D†&ö¶?ïÝ*Œåê?k['FÄ؈?`nËæL'?]{ýx¥{û?bf¨'ìK?`ÙïîbB?ïdÚÿ¯<?|Uö?{Sms4?rÉÿ'?‰‰†q¶¶?u$Z÷¡"?ïß`dªá?u"àYiü:?elÔRöǛ?q04œ.X?Vñ–¬9Z?`L†4vAGN3FGL J1424.3+0434@uø›@-¹@M1πsÝÀ:…Óé÷€À;Ê(X
Þ¿Øñû	öùÇ@½Ta$X@㽀~•‡¿Ý÷›ä…È¿çñsÛDî¿åh†0ÂQ¿á¼e¦ÍߜAGNbll?ïê´jfŒb?`)»3
?GÚó"n?H·ªQ°¨-?^©°ÿ˜ý??Y±ÜM‹?ïšh"B?ˆ"f~o?uۗÖvõÐ?v)eߗÓ?|ðW!ï"ì?'¨ ²'ç?î'(,:ñ?ÙGاc–?'Oùˆ.Ǜ?€üÄ{¸d¸?›‹²IÚ8?"²>§–?îýÇLŸ?''‰»?uˆSYLµ?pñ"—X?šëòG~Æd?Ϫ§ÒÐ?ïù£Sú?@à3vlöP?1#k
oö?3=~XÜÖ?@àþqåW?8Œ>Ü´ç»?ïÞÛ§?jñóDR6Ñ?]»âCz??Z2¿¦ŽÁš?bFgŸ¡Èt?dÉ/HÀ?ïk·0ª?vA­´U ?€´ÆM±(¡?ls6€]?"Šàr–×?hùÔõ"±ó?ïÐR -Sî?i.½ÉÌק?Ux‡Ñ9g?Eœ-[ZŽ?rxá!¾ý?g&PŽÈ68AGN3FGL J1424.6-6807@swp€0<ÀEÔÀH^À8l›
²áÀ;/*Ê®å?ð>¢ýñ]@{L‹Hóå@I½ 1xÉ¿ã1=¦9÷.¿ç-³;£'Œ¿çÈoè<·8¿ê™¼å¬ :AGNbcu?ïÖüwÏU?k¦
`/Ô{?e¿œ–ƒÏ?acÇ»Ad?cüȉbg?_¨áE?Ý?꘳)&ƒ¼?ijtõSk?¤Ö½'p€?§¨•†?À™ý­u®?Á™FÁ
/?í¸9›"U?š,ڃ¸"ƒ?¡ï*8Æl¢?ÌšÖc,(?¢<OÄ×?ëõ;hÒ?ꕹ!– ?¬¨âB(?©3ñÁpD®?˜\u]
ƒM?¾¸>'ÝE?«hùõ?ïé!zµ9?`;ù^?\)l`R‡?Vãt¸O?Q"žšï¶Û?Lƒ•àR¦?í¶Ztbû?´4h¥Kx?'œ1Ê3‡š?'¨³+Õµ˜?«L?Ò0—€?°*Î|¤q?îû6´"i%?‰Ë" èã?'às
c±?kñÖ÷'?r5û°'4?|´I3RÐK?îM?x]V??'o\ò-á8?•ë§[ã¦d?|³Հ=¾? 64ÎÌ}Þ?ï`覆¸AGN3FGL J1424.9+3615@O¼ÿëJ@Qâ (zÀ9]Ô´øš±À;¦V6mzWÀ48éU™@UòŠ÷jZ@ÄÓ_ãëL¿×Gž?È¿å›ÖDg/†¿áaÍm-8¿ÕŒ8ôΖAGNbll?ïòêëh:É?Pӎi|I?>"'lnï5?3Ô𮐎?R‰Óùʃ?Jú'Y's?ï³Ø·¼šP?¡.¡¿]?fsLš§>?m¨Í&Ùoˆ?zÙþ̸? ²¡:hTÕ?îü8EÒÙ?‹|JשD"?ŠJ"úS†?ï²½Èq?"GG됭?'–âBÊfÖ?ïê®2"
$?s˜Ë;pÐ>Ä¡Ô­òª–>äõ¬ÌhÒ^?eL¤åz]1?s˜i;_?ïúy¸u]?8-ÏAw‹ù?21A}"?% ˆ2¬a0?:$¤
ÂÕ?2«BJ?ïê9xWæ­?mý¶WHü?QÂýKˆÕ'?S3)›ÑX?YÊ'ðº?hpoCü¤l?ïŒô
i±0?t÷Ø?{`¦~œx?p‰¨ƒ?Æ?~"˜˜ú´?fòÛ³$D*?ïü–ÔöÅw?N‹ªÝ;H>vä9æÒ>¦x¦€<,Ñ?;G÷¼jÏ	?N‹ª¯AGN3FGL J1426.2+3402@LÀŸ¡ñW@Q ß@wÏÀ:R¸S™HÀ;áðT'QÌ?ãÅ-žÉ¯6@
SÛ&Éï?þÞ%ÀÕ?Ù¯L+§¤¿ß Ëkg›ß¿ÓeØÍ¿æ2¹˜½|AGNbll?ïébš²{ñ?aØÊÔ?R›Ìé
¤?U4vr¶|?Zžý€y°?TØ).†?îgü4:ç?¤b'""7Š?šzZ³+›?œ·œë©4?•ƒæUÛz?•ý­Óñ?îôïF'	b?‡Ûýž$8‡?‰ìîÿrS"?vëÛ2¦¨n?"kŸÂDáñ?ì$_yn?ë¿~˜êС?¬=Õø•^"?²µE˜5?¥±Ÿs«?®Œ:²ï±?¡­«å;ü?ïÞ½ùÜ`¥?ªsð¦fs·?k«çV;M?ªx1Kۃ?FXzß@o†?A"pÅ€?ï"Mê; ?‰QѾU?'•<A–¤¥?'/cgòm?x®'i—zÞ?x]j˜¿õ?ï{ˆ«¤wÞ?tù=²×Çì?}[ÍLζ™?mÂ]&Þ{u?'oî}‰1.?gEžXáÜ?îpOå+Ïx?''7&g/Õ?¢»`/=ûÑ?‰^ÒÅˀæ?ˆþ…þójº?'
æ4·HªAGN3FGL J1427.0+2347@=}z °P@QúÿåþÍÀ6¡H2ž¸½À:ÁÅìß?é×Pô0¶N@d¬Iõl~?ûŸD®'û¿ÖÝÕL'î¿Üãȗ3ó¿Ú#¹m¬<¿Õ¼aÛ(AGNBLL?ín–#ÿtÑ?¶¼J8Qbñ?d®³çœa?fðPÜô½?³åÙBŽáS?¶[ÄH…/?︈9ÊÑö?¯ý"µ¼Ò?n;âðÀ?p¦[õ²?tU¤¼˜»?y?õ«–°×?é̪r§4?²¦˜JX ¥?'ÎŽ¹ƒÔ<?‹RøÙÈ?ÆuÃàϨ?±n–64[?ëaÏÚ.›Z?²0}9‡M?ieÔcx¯?n	×aK8?Â)E§1»?².k¡òU3?î]ÆÿD?­äŸ‹ÒÚÏ?`n¹w'M?cÔi&Ò2?©£âŽN9?­^¥…h¾?ï⻢
´í?i¢¡KÝ؝?Y6h‹kª?VYèÇ=?`©*Ÿä'?c™|ºÑý­?éO3sÂ?µ4¦ñŒn?–·5/<?'ô9vŽê£?È{%Y?³ë̇\?í¼úîâæ?¡¼Hˆ>"?gν-©Á?_Ô£nyAJ?±Y²ž¯J^?€¶å(AGN3FGL J1427.6-3305@tRÕàqÅ?@9—3 ¾¼iÀ8'ÖJúÐÀ;[Êò×ùQ¿ÔÚÍÀV‹—@»66ó²@XØ\œ8¿äB2øOÝc¿æ[k2þÚç¿æÍõbµ#¿á|RAAGNbll?ïûé	eѸ?8Ô«¹×Ç?&ŕ}·b?$'ïû"e#?5°RÌÚ´?3Çß6\Ó?ï´S—Ï?‡˜€/‰\??po‹Û˜P?'3wvv¯?uŠJ[ïÆ?xJίIà?ïKíªÏK?€@€¢¡…ï?O@îÔQÛ?jæC›/³?\ôÝP?y&'"­?ïÒ°£:F?q—®–®"3?!IýwˆÙ%?%%ž»\?v^Uºãf?qèÃàÙa?ïþcȧN8?#ç/ksô?wŽC>f?Ámu"\?\œÖ²?b²55÷	?ïã%=@4?hËc4ꂿ?W'ÿžs¯?S<ð×÷?aC/èÃ~?cv"ñdë?דּ–‰³Œ?gQ"I±û?q*¿ÑіN?\%ÊÎE¡ã?x{tõ³;z?^¼
«`ë?ïølàþÝì?Mš$Öñ=?J³S~æð>ýÞ\['¤
?M7Ñ£õ¤1?Mt‹öĔQAGN3FGL J1427.8-3215@tYªK@:W– hUTÀ:apÑ#s£À;±,±8ò¿Ë¯iU•D@¯~瑟$@I¾×ü?ïGΠ·p¿à^–%›Åï¿âž:Ãu`)¿×X
1/¼ AGNbcu?ïïâj\®ñ?TrÕåñ?BÄs€9ž?:Ü\"sAé?VÙ!Ð"'b?Qv6ýI˜?ïxÇȽ.Û?™óW¼Y«ü?zeY¥%§y?|9oµáù?"›a§wZ?•~{íXä?î°"c…$?Ž9c'yÛ?'lîW3?†JÒÞ ?—nGŽènG?À°ð/uâ?í˜ÁrPªg?¤ËÉZ'ó?'Öt}•?;²ä¾c?°ß%ٝ."?£ùr"BI›?ïÝf¼?­þ2YWØ?nˆí~bü?®ã^M'?BEÂ8Vôu?E³ÄaE«?ïχOj!?}y˜•¶&Â?f	cmÅû¬?jOOS³Z?jÙ90ûÜ?vsÕÔ¨?ïa‡>?Å­å$3E?'Š÷-e?zHû8_‹?…5å9_…?ró§ßÜä½?ï|óžGÔ*?€î³DÅÂ?dÈ¡õFõ?Ur.6òIý?‹ð:«›¦?€qy™cßAGN3FGL J1427.9-4206@t6m
J@1Cƒ`r0ŸÀ6p`w	LÀ:€®n<ô}?þx"¹7Ē@ ·…gÞa@⾛ܔì¿ßRØȌ¿ãÙù·w·-¿ä±¤0Ëпç«)>gĵAGNFSRQ?ïå]ŠIÅq?b²ÌÌóøY?NŸÞü˜­?TK(x<M?bú}øóW?^j¤C­³?ï©8s—"õ?Š§y$Z݄?ncÃl¦o_?wap·Ã?|1äl¼Aë?†+ÓdãÑÃ?ì$tG5Ú¿?ª·^.<1?©mIJ=? 'ÖB'¨ø?²%¹!²ì?¢w@òA.&?ïëcÛò"—?r­Á'ÞŸ?•ÜØòZ?I0ÅŸ~¾?c§tï-Y[?qºÈݎÄß?ïó'Eåž?U
Þµ=s-??Í_ÜAW?HJAz^²V?Pên¹qÕ?MŽâ1_U?ïà…k¶?kÎ~fWæ?X<C6
h«?S"Ä ÞùF?c\À•}­?eÝ°ŸmŒ¬?ìÝÐD?«8÷ ìc?­FDhÜ
?¡œ•Œï'?°³îÃ7dÖ?¢€`³UÄ?ïü	WÂÆ?Qƒü–—p?e³
sia? '§`C'?<JÕ`Sãn?PàL`ÍiAGN3FGL J1428.5+4240@S^<Ö_@P93À9KÏf@×À;>vƒêÛ¬À0‹áu%@W]ª*5‰?ù1¶@™MC?Ðm=ú¦=±¿ÐúMƒÁk¿á
a<…í?ÐLW
l¯AGNbll?ïóU庯i?Mg'y][•?F–=Å}??@ý!±‡?L¡Ùmœ¨Ü?EÎ)vó?ïɧk"Mª?}1H¢[4.?gUR"ì•=?nóe~94ã?oA­P»?r'JÅ<´ã?îº&¶vW?"PÅõ€Ô?"Ö!CÎ_??Œ÷Hüg&ý?"åõûkÝ?…Â"¼Òà‹?ïß(®cÄå?u#@½çL>Á›®.ÿ¼Ò>ÐxM½"?piuank?u#%-êԊ?ïùéçÿqÿ?9Zžõ_¦K?9zÂ|ðÓ?/rñzHQ?75ûèûñ
?0,$´øå?ïéèâ<k?ddXC‰ÔÂ?Tª¿wŠŠ?U€»¥É°?W";†>Ù?XäJ¾m?ïIó¬¾0?Š=z¾ß?‡×ºÞÛ¦?'É~Tc?…«YûíùM?€ËµgTr?ïùñuΎC?CŽµýâË:>Œr©ýjÒ>œxXÛ\?H8`ðh¹¬?CŽWï!Š˜AGN3FGL J1429.8-5910@s´à&Eå?õ ¿ÉÙþÀ7(g  ‰xÀ:zõ‹1÷Ê@wÿb÷*@ßaÏÓ½@†Ûw_ˆ¿Ñû@VÿŽ¿ãoÙU¶Ì¿èP]<•e¿ï	‡Q²>PSRPSR?G•Ö5l?G*6⣤d?ïçàW ×?¢£nì²W?›ªgQ…Ê(?¢8HÍ¢€?7bá:Í1Ã?Z)=@žDë?ë«8°u©$?´@'ªÞ?ÁGkÍ61É?´W–ànÐ?‡pLJK_æ?%l;½p?ì'aÍ$i?«Q6¿Q?»ÖÞbe>¸?©[o€UÎ?\lœH#g?VC¸Ô£Ø?îK—ßÛ?—ÅóºƒfU?ªlqžL ?—d(uIk?<‹§¸ž#?@ÔlŠ¥uâ?îÝyK™Ú?°T‹ªeG?¡ïSûÎÄ©?°Mè؋?I㶗¡É?_­æ²<?ë†	ŒÌŠ?®åЅ½9t?ÁÍ÷ã.–Ÿ?®øE»9ì$?"=}™EÒ@?7'Uü®3?쌒kc6—?¦·ë犷U?¶Ì
<ݸ?¥
òºzÃH?i(ÍeŽN1?[D×[­6?îMð…°ûØ?'˜t—ÂÚ?©ŽjÐ#0–?£ÎñPSR3FGL J1434.1+4203@RÄøä@P^ÀW¦À:4ûŠOzÀ<'~Ê
{¿Ù–Zê%@m÷êï]@"í¨'Ú¿äÐX؉C‹¿ã%8~‡×¿æÖ&'¼¿çF£¦@y AGNfsrq?ïû0žÑ??:ƒx_?-T;æêì?,=òú"ùO?8ýß=¹†5?7\hƒÈ‡#?ï±ö~Ãv?­°AÆÏ?rObX¯­y?tP"Ræ¦ð?tµ^q|{p?yMºt
ãç?ïWN
zy?~ˆõаÀÕ?±>ô€ôž?u¾
ñ 
á?ˆ{>\(—E?qÅlÇ!¿?ï¨L}å'?€"úŠ·‰Þ?g"$|'y?c¼ˆâ]Fô?€hSGó?}›rºm0Ó?ïþJvyaž?-3HÊÛv?Õlr,˜+?×é5o‡? mä"ÌÆß?"w‰2õôÚ?ïâ¯FÌd"?eo|¿! ?ZpxD&£í?Wy|,q.?`}=ƒV?\€þn5·Ð?ï®%a…ÎX?qbRA؝Ô?rÕVûæž?j»õ¹Q<?vøF±•é?dÀŠßÃ{?ïò÷'Ïÿ:?YþgÓ9ªœ?>}(mRµ?0ÂÇè¬vÝ?Rq'=֌?XÒç—ùgAGN3FGL J1434.6+6640@[a¿7¸Ô@G±K¹ëÀ:µ´ZæÀ;õãåî¿ð(¿1-Êi@
Rß3›Ž?øCú€º$ª?Ð¥zbò"†¿À»iÝ=â¿ÓIáùR¿Ç7Tºc±AGNbcu?ïì3¥]{?eãÜÛN?9ÖîL´]?6ú'U¿žÛ?`' ¶þ^?c«ÞçÐÊ?ï¸yˆyƒ?8»,AI?m·æaw'?o`®óö?ã?tçH´ÞÉ@?zhÜsò?î'HotF?–óÇê=`?"Èqx‡3?ŒÑù'5Þe?šEyŠD7?'-Éa¿Tî?ïÆï<¨?sîC»#֗?/Ƽ€æý ?3¬' e6?{ÿÒi_I?s"È\Ä2?ïí}dPê?gÕ¦â˜Á ?0±¬:GP!?0´|Ÿ](?`leÐߗ?g1ÍðrË"?ïæÞ
sŽ?eXW'U¸!?Va-§æ?SC$–Ý›?[â¸s-Üù?^áVÛz­Ð?ïÑÃNY?"›žÚ౒?Ž4jO[U?‹e°ºk?K'ihh8?‹vP	é'?ïö]÷íÜ?Hû+¶tÿÂ?'°/©?åٖ; ?R3™ÂÂÕ?H™ägPÃAGN3FGL J1434.6+1951@5`àЏÐ@PS ÒH7À:0qŒ4VIÀ;q°-YÕ^¿ùu¨6À[@RÆ ‹;@ûõƒ¥¿æj²Y¾¿æ×Îú_¾=¿Ó篧"Y¿êR êNqAGNfsrq?ïãäŽoß?főCI?Zô"æÖQ?Yü¿Z}·×?]C3%…Af?[ӀÆfÄ?ï§m=e!?‹S|y¯5¼?tvéÛR?"¡&M>·?wҋo‹±U?zQv+¿9?íù¢¬oé?™"«á¹?/ Ö?ÊS³¡Ñ£?¡Ñ±•?45AåJ?ï°"9,"?'Qä?G\#úàS?K•VÄ'r?›o^E8L?'ê*óÍt?ïò;w-¸?[ßf9"G?P¿BßÇP	?T¡Q%Žé=?E"ž­|w?C²'fk?ïæÎÞm¢?bÝW±²2?V½Î¯‰p±?RíǜøÐâ?[¤uUªè?ZN‹ÉåKP?ï©¥!Úh?_\L€7þ?'pjõbf?ŒqÌöé*ü?ˆ4À×17?w€†79°?ïʀ*Ìv*?kBÌyí?('è r?#@²¡J6‰?yþ²zo¤?jî¡!½ïAGN3FGL J1435.2+2023@6¬ ŸGX"@PV³`<ÎÀ9µc¾yåÀ;ByÙె¿ñõ[YBœ@
3oЍ@oU ›k¿çž3däå¿æè0-¿Û¡O–U¨¿ïÿ«mâgAGNbll?î÷¦2ëJø? GÂÏÜz?"ê•_£(º?"ÕæPÃb?–•îòÅ˜?šEF•—¯?ïíªN-ò?™ó€ã;ú?EPäkq`?WyŸºV9?‹¹óª|ØÓ?#hö?ê8gòÏã?ªc6ßë?¶Õ3¶U? b;±Íf'?¸i	
Ve?¡gøIü…?êôåîS?³p<ê÷?˜À;m4#?š˜ñnÙ?Á,'½Ö‡-?²¬k©Î?僚ÿÜ)ó?ƒä×ýwÐt?pÙAmê.?qzX0ü È?{Ⱦ¹þWÎ?zd
x¸?ï¼Y9N¢?€o<;¢ä?rEúŸf·Ã?s­$"5•Q?oÑ|.Û¨?q"1Ñ_?íÒwí³ˆ?žXÖ"9zp?ª{7—xT?•¶>÷Ô¼?£ç¡`³*?¡2Ì"[?î|¸/[ã+?•Í †ù¨?s¥#¥s"î?nlP²¶PS?¥¿Ø"A :?"Üá!U€´AGN3FGL J1436.8+5639@Xp6ßû}º@K'ÿyÈÀ9÷ ·›`À;ì±AV¥?éÜ»¤¨¹@ïçÈ{¯N?ÿÂ\@©õ¿åëÌ´¿ãÈ|µLs¿Öf÷ŒO?j¿ÑPíè®ÞAGNbll?ï¿Qn݃S?:Ú7?Ptu9¿F®?PèdQ¿Ž?|:+U\h?€`øéåO?ïD«Ÿ;Ö+?œÇÏo»æ?‡eZ…"$B?"5AÑÈ-?‡o½®õìï?ŒåcT_¿?î°ájZW?ŽŠÊf¢^?‹[ÓÓ`ÁŠ?wŒúáõ^U?œ5èؾQ?ˆ¼fóá?íΘi÷H)?¥es:Höö?š©.‡ÞÎ[? ­>$‡7?¥ÁâœA?™‡"IØÂù?ïîٖ×ð?`Պw›ú"?<°S¦ï@?6…n¢-L0?[ ½-Ö#¤?^ð|1XWz?ïÉFmL´?€¢ÿ™?k¬ý;½a?x†TÂI?k
wäÊcÌ?qæXzç?ïrÀa©?x	Ø՜d²?{óåž_'?i°tBOþ?…U-',I?p;†€òŠ ?ïR7Š'X+?ŒÔ»EËB1?Œá ˆ 6?†"¦4w9?} úÆ5&#?ynî`øh´AGN3FGL J1436.8+2322@=ÔW?ö@Pzd_ûéÀ9׎¢Å'FÀ;¸"lá«¿ÔxlÀ?9@ï¾v@B½ŸˆF
¿ä*Ic4¿ç-žÂ+Ø¿ãL:'K¹¿à§Á^&sAGNfsrq?ïù2‡'¯?G¶üÑ ?$ÊÑ"o?!Lì>­Z?F"²1±Æ?ET!Eþ?ï¼fÊS9¨?€|¹é*f?loúudΑ?rN£ìv½Ï?s"~$!?wyËkl?ï\œ¨Læ?€1Àãþ¡??yÔÑ6"•¼?kPÝ~zù?‹î¹B£¶?yq;É:"?ïŽØX?€#TçEn?V~ D²¥B?Qƒ¶ªâÇ?‰z$â¢?1—'Q'œ?ïý:ZfJY?0¨µÍù
ñ?AÇ'²`F?@=ÈÞ±ï?.¹s¤-&$?*éùvA ?ïæ3	ÙÚ?eH"pÉA?VŽ,@ä@n?T-tÊ-¾[?]
µSrŸ?]쩺‡|?ï¼ÿ9RÿN?c2'8~L
?iàæ}C?WAŒyäà!?t[ôoÃz?Y´\0âî?ïë
í©f@?Zà'õËÊG?;àKI4?,
›Àxä…?auþ·èþs?Y&<W"®HAGN3FGL J1438.7+3710@OÏ`?Û¸"@PQɀ2WÀ8¬N¡MÃÀ;¤ÖR5W?îÅ9oý@k0¥F@êÆ?iøA¿ã+ñÍ[¿æwè­0­Ð¿â'^³®\Ž¿ì÷=Ûû
AGNfsrq?ïø!–Êÿ?Dº U¬0¼?D",ª.?@¸fè$?6®ï†
¯7?1ÁÆðÓù?ï¿ôs_?ƒüqӞw?lúœ¥¥?qöG÷?qˆ£#oiš?s?KTõL?îçQÊ»ƒ?Ž2K!~Y?"¿'wwŠð?"»ö^î,V?Ž¬˜^b	U?~uځO"¸?ïå%O+ ?r"k—Ô£«?Dg­Ò(8±?O™íT*·Æ?eÀÅ\\ùˆ?q³d:k?ïú¶SûD?;ÕsúÚÿ??æ©áÒ؆?7Ñöó?$Ò$›"ò?Iú«ãÒ ?ïäÌ"á_	?g–\kò\ ?WÒÜ,ýiA?U'',F;Å?^"Þ9Õ-?`rF"Ö?ïQ–Øôù<?€žh¼$.™?Š¶k#žòr?zM´ëV²?€ãޘór¦?j‹V¡&Ÿµ?ïûiP>¡?Eçab¬2?/¯h=
?/ë×5Ò»÷?5-7Rs®?CÌ?6¶EAGN3FGL J1439.2+3931@Q2Ü¿ôw6@P²-LiÀ9ç:Þ"_¦À;Ÿt´*¿üBÊry]@Ѐ:øÏ_?üU«`@‡…?Ê^ɼ–ò¿Úä^ä¼ØŽ¿à†8<B·œ¿Ð›¦G"AGNbll?ïÚùؕû!?qˆ×Ðòz?Ee£OZ ?@Nÿ,Jñ?o¬¾‰CZ?p£iÐHðC?ïÁ‡6#?»QŸaß?kR÷n@
k?tDLÀ_ò?qÕÀ»˜Y??vC¯o«FÞ?îüVÏçÖ¶?Š˜é¬'«Ð?Œ³@¸«o?€L‰Ô&I?'… ˜?€8lzÛ?ï¯OýƒT?€VOHæÄ]?"'ÚÓpE˜?'hfˆâ?ƒá¹=ÚÉ=?€C×/N9°?ïòy)a£3?]¢Bsæ¬E?3
ÅvûÜ?+e¡e¨5?VJ;ÐÍË?\`S¾P?ïçÿ™jË?fnٟ싃?T:‰µ¦"?R>Ž'íT?[ÆV1)3¦?aþÝÎ"?ï€u<±Ðâ?{KR§€V¹?7Ïq0×?s¯\¼}ü?€FɃß?m÷Ù}д?ïñéij/?RÑ_ªÏv>ôðY¨4ï>õ¡ýûDL™?[Ú=V3;?RÄ!êJàôAGN3FGL J1440.0-3955@tIñQç@2X&NyáÀ:MJ4¸À;¥÷T_Ó¥ÀrƒSÜöæ@
¨Ñò%¡Ð?ýÒ
ÿGv?ïZ–¼
6¿ëê%NÝÍj¿Ù#N§ƒ?R}!$#1AGNbcu?ïå#xU&M?g¶üÃ>?#'+ÿ
C¸?"²TnP¤=?i£e-×ز?gPïjá<G?ï†è•¼P?–†€Ç—'?mH›RÀçó?p!)bP_o?†ó³·8M?"®¨ú¶?î™K@µ?'µÝn›ï(?†è-?B$?v'üþT? µùš¦®?b;
¼
?Í7z?ƒ÷­ç¾>ì¦w=Â?>üáãþñ?ˆˆã)_¾º?ƒóªêf…?ïöUú)ô"?Në­¾¨)í?/àý¦Ò?}š^]2?Qa
ל+?MÁ»…kÓ?ïÜHú+
?th}—ÛSx?W"ŒÉVh?X€¤1 ×?gð<,²"?pÃî›ð\,?ïQ¯aÏJM?'Êê¢à:?zÀÂT-;¾?fZ•fM÷?Ž3ÆnpÒ?['Úî°C?ïð•\{´Š?U0ƒ"E&>Á)$hQï">¾¯Su
Ž?^̱ÿ)?U|àŠAGN3FGL J1440.1+4955@UûÐÓ@M•ƒßóðþÀ9¹[O7À;ó¼w¯d?Õx æ³"@c0¦æß@Ð^à
AL¿çuµòžK8¿è®€9²d}¿å åõ"¿Ü+µ×NJAGNbll?ïò3Rܤ?V^¥"×£?PZï"ìÄa?RQõzôÈ?F}è[œ$Ž?B*X¼;å?ïpžY›8?"8–°«?''5T?7ÒQq"?Va0}"'?ƒ¬ìÛ&¬
?îËr[3¥?‹ï°à.¿¶?Œ¤ªê…â†?{‡‰x˜š?˜K¼Ah#?…˜
1ãü	?îNm# ?£"*¿¨>?"…çsÖá?'Òûó¨o%?¡V:òŠÅ˜?=#ÜZÒ?ïúR)\_?GYÃCJÓD?<(Ȗÿª?C»›VLå?3̤ú¿%G?03ׅŸL?ïÔ9£µ§?t8Â#.ò?fåË˔?jk ÙÃ?dáZš¬?fvј6‹¹?ïtùm®s	?{Τºn?}˜]"Õ æ?nþ¤éY?ƒõuùF?u0$ՔH?ï³I¿c‡?};§O?tœXŠ3‹Ð?f›·GQ¾?q¾È§T'?vvKh¸•þAGN3FGL J1440.2-1538@uÃ?…Q
@Cßcߣi&À9§%?TªÀ;ÔCéd?ÔGÈÛ?p@¤BQ3Na@¾@—õ«¿ÐÆqO3Ö¿étÖޕïb¿å _ƒÉ"É¿âÑ,¾'ÅAGNbll?ïöÁ¤
òÞ?L_ø<x2º?=Í¿Ä£í?<˜âPÝ?FŽï7Øú?D—0Lo•?ïrâ±C7?'ÀFNyè?}°y §';?€…ú`ë?"o,Dì?Œ%ÚbÀC?ï€Ô.sŽ?‡U¿èee?‰n5™
Þ?{÷Ÿ+Ò]Z?øÊæõkG?e'þecA?íÃÔÿ—X?™¿;fHäi?ˆAº¬Ü?üΰ[?­²Q(?"û?˜yü©?ïûk?4?Gûñšû?0gKyCÖ?7L‹#Ø?4@ Ú²o±?;—Óì -?ïÑ 
5À?tÔ`sîôD?dÜå?%¬ý?a´"
ž\£?j
ñ}Šµ?p'D›Oy'?ïŽá¬z>W?y™i5Š8Æ?|'$_iGÆ?q%²ZÙ?|
¤X˜?pÃ¤Uõ?ïu'i"?yßo7ï{?sî¾jxÁ?\f_[ã\-?ˆ¨½áô?vôCÑqAGN3FGL J1440.4-3845@tR̟¶M@3ZŽà3·À9ÔuðG%XÀ;gš'Í¥:?±Â™¾¾¨X@Úf¸ñ£œ?û±^ûãç¿ïÏ	XU?æ[éö±Ö/¿ãè_ zù¿¥{1‹a·AGNbll?ïîÿ¸Ã'¡?Z#í×¾?HˆKOëð?E¢zÉw¬?U¼ŠÌUL?V-?l<p?ïÉ¦tò?"TuÌU›¢?s°až3éÞ?wkn´ü<?'5e'!Œ?_SÞµ"±?ïPd"Ë?‰=ŠŒm?‹d½ç#1«?üö|ãO?'Ý·»%È?}%ñWûÒ?îýZÂÎ?•Ï­¶:?~È£\&?ƒ9ïöU?˜¢–]óýÉ?"›Î6¶Ô?ïù1´zgò?F½À Õ×g?1ÅÃÒ;Í?+]Ÿ¾"ß?BVLÿiWŠ?C'ÅÏâ¿?ïׇpü?s'0­{0?\«|¢øD?T^¡MùK?j#[À§©?pµŠÎ%Û?ï"´"Ec?xo鲌µÖ?}Š²E>)?q޾Ϥ'œ?€9¹ÐìÐ!?nC$–	?ïÁ˜¨FÊY?pó,u½f?ZO¼)‰4Ë?Nߤš›xŸ?xŸ¼ÃÊ*•?m™¯›9
AGN3FGL J1440.9+0610@vq[«–ò@LKT´FÀ9<¦9»±À;–g¼§»›?á¦9xzBÅ@Ý¡ejè×@úEà4Ä¿æG®)ôp*¿åYø/|¿ßu`Ôí¿Ø–Lgâ'\AGNbll?ïýAÅOÞm?+Áµgî=? 8€x‹?uÖË('?+Ì»ۖ?#§~À?ï±,2bþ¨?·º±?q¢E
©?r'}ç˜ü?uÇ¡ÍOS?y('ŠÏƒä?ïwÖ»¸þ9?xŸS¬Í@w?wP`-?cÀ"˜j?p?†bESøùÇ?s­¿¿;Ë?ïUkgŠ±R?ŠÅ‰åÜ
>?h¬'Á"'"?hIzÉPÀ?'=Ñ#x?‰dj°…/?ïþžÈúґ?%Ü5)"[l?¦ØI£K°?
¹"?€"£\h?$HÛõ¢¡?ïâkËç/á?fééðˆ?[\'º›´‰?U§÷È|o¸?_ËÕõv)t?`Âa$"?ï½BSÈ?hKÇ>Ævá?j3€ž=»?QZ~ç?t^ñ…?d
ž¸¼?ïÜtŽáôk?fª&¨²¶?WÅ{[«Km?H'A3|Æ?g¨³e7/I?dKÒÝLAGN3FGL J1441.5-5955c@sÅ>€8Ÿ"?¨{϶ŸQÀ8j3àØŒÀ:5é$h;?ñâãd"Ó@…ÝÞÂî}@x*.¤¿á£º"ˬ;¿ß_[61•¿áû Ôvd¿ç/z¬nˆtOTHERspp$?š'</Q#?—h6J>ès?¢Px¡þø+?¢r¬±( k?î	¾">ª¤?©÷Àcƒ ?¤êzûM±?°.D?òs?°¬Õá?µ"« ³1y?ê/¬ZçW=?¿DÙp@§1?Ǎç8š?®X;à"Ä'?¿·ÁYÉlg?¦Bw«ñ?æF$ŽÍM?²Ú¶1K?ǒ^Ôn#A?¹¢K×µW?¸`T	FĘ?¥å8ì{V?ç]ɒcM?¼Ì5HóJ ?«¢%­"J7?±Wa±bóq?¥;nÒ+í€?¥ã&ÙÍU?ìò&·é¥?¸Œ(TÎ\œ?½@e»É?ÄFB"‰çö?ĕœÁ¹•°?¯äF¾Ï?ç2˜cc§š?Çgvø–ˆ?Ó*¬ø'Cx?³%"N>?½ó3F‡˜?£ì¬B9?â¬Cíþ1?³ØZ±$ÆK?ÐP«•=?¼Jêp1ýd?ÃÔ®©²R? ¤"†uª›?ãµSMHÍ?½ÞN ì¬OTHER3FGL J1442.0+4348@SC8€®@Oû¿ÿ^ðÀ:R@|ÇÑ»À;سc$"?ìȨƒu@
µ2g±??üyvèÀ¿íÖÚâå?¼Ñt|S¸¿­).ˆª¿ÝØÓ+ò³MAGNbll?ïÜq'%?oív'÷?WI›À+?R¥½s¦[?gê֊c?lj§PU?ïE:µï¡Ê?'ÿTŐS±?ˆÍckLc¸?†nìïBs?…ãï:ź?†Uì·
1?îÈ "s±?œ½¨VE½í?œKNÅÑT?¦Ë¥o!?¡Í֔ÐÛ?'¬M:[¤?îJó&[g
?£H«ŠDØp?žÜÝsàÏ? "£o.­?—ĽǑȗ?'eBÃ(?ïæxz:-Î?dÒdki¤?Q?¸k-­Þ?Kmƒó;<œ?`穃ÜÂÞ?`mDrOó?ïÂô7¦­?x'øŠõ¢¾?ph´ŸÎ?oNÓóó-?l:¸i?k¼%6ҙO?îòƘ͎5?'ãÿ±`µ?Eó<=Â?ƒ‹"櫱y?' 	ñׄr?‡'ñªiÚì?ï&lèOxþ?±¶"Fç?––@å¤Ö?ŒV­û#Ã?rpˆ$èqã?hÂõî75`AGN3FGL J1442.6+5156@V· '½´@LÌûÆnåÀ:ÙPÑÑÀ<™‡ûâd?åG»ÞgÿÄ@
q¯ 5w?þ–?ïX¿ïýÓٗœ¥?ïÂpdÞÁ¿ÐͰý뚿ê8Te†(AGNrdg?í®êL˜?µU	j¹?±lˆ©o@#?µ:Ú?f?r1€'ó?rîÑ
r³?Þ Y!…Æ?Ӱ֐ߥ†?Ý™#Ž6?Òô~°<ÑË?³«â?²Š¸ø?ë¸>Íñ!?«º˜@ê[?¹é?½7á÷?©äJúmo? ©"žÄ+?Û4ý4_?äÓÊf"Þ?Ç[äj«Î?Õb?вò?ÇcŽè2F?ŽÅƒ¤²ì?o@}
Ò?îÚÙ/[¸8?´¸ó>5!?¡¶ÝQsH?´a[ðÌg?db§U$?i…±¤'?é¶}Bg?ÉeGXþÊ?Ľ¾«»žì?ÇEwGN?¡¡5O…2á?¡Y!648?íƒöžq3Ž?£ˆ5›§Â¥?¯»6æ/Å!?¢ˆB›e^š?
¾n	û?ƒRƒð	ô¾?ìÆAì>I?«–F§$Ø?¸ºáD>x€?«L[Śö³?q0õ­JV?mç¾¥£AGN3FGL J1442.8+1200@ ¸G '¨;@MéšÑVŸÀ9±Ú/‹ÞÆÀ;|1u¿ãy:M¦ƒ@^ŠPPzl?üºlà¨÷°¿çyqcªÌ¿ÛvI³ç¿Ä\qî¸b¿Ý¼ü'.¸AGNbll?ïøíÜ´Bà?@»'H¼l?4•¹L'X?,º«êå?Aý¯íüS|?:u®dé'?ï´À& P-?‡ëqÂq?qFڛÑ/?':6û\b?tYÕ+é"h?yW'eÞK8?ïa{@EÈë?z⥂­-C?M®Á?l$?o­˜3îe?‡úXŠÖiK?qхiv?ïS3ϐL?"A¿½@¤ø?JPð–Â@?Ly¿®èÓI?"Ë'0Æ?ƒâç&˜?ïüŠ°{;?2ˆß_š?(¦}WÒÔ?%=Ë?.®|*Ï¿?&5Ì<yJÔ?ïåÀ]A"b?eê(,åÖO?Wšò	ŸGx?TÎËõKÆ?\äSE4ú?_ʦð*Þ?גּe?luAï8[?r×LQÅ?b­"ƒ£`´?w²»'?_è×çRu?ïÖ>‹+Ú?`B'?ºœö?;{°ƒ@ä?-–Ž':?s/''ªôH?_Dˆ A`AGN3FGL J1443.9+2502@AKy@]¾!@P,rßñl¿À9D–¸=ɏÀ;š÷Ÿnd¿â/	Ì@ø¯.+aƒ@V¾|'¿àEËE…'ž¿æ(>Yú?¿Ô!Ë4yã¿èKŽÿaÊAGNfsrq?ïº;·U/?Šo%‰sÔ?cyxŠœ?lXë	)n?ygžüƒ>?†Œ&±žá?ï# *ÑÀ?¢/í‹qš?‹…Ì¿(!ò?—T¼HYÛË?‹²(±¤þ'?'rªœ•/N?íiŸ­H½?¤F
#«¶?'¦â¹»J?ˆ²î‰é"?°
rpÉ?£4çfå?í±†º÷?£dÞÉ?ˆ¾?‰µÛáÁO?®æ›0ñ°?¡V>R°'è?ïé Å)aÆ?mò/¯Q!?QIŽIvš?Xã Ð÷Ö?[ufc«-è?fÏâ#É?ïÂüII?}"Q.€ü×?o¯üѺë?tŒÕdð _?mSåòðóR?jÌåô€â?îÚ)åÑß?'ZšF¥œ?ˆýŒ¥mÌÝ?"
@ÆFÞO?˜<ɯ¥¹?ì*—è›?ï€Ö¬Êxà?~ÿè%>c?gӝOGm'?`;8Rf['?‰Õmp ðß?}'	çÜßAGN3FGL J1444.0-3907@tZàP7P@2¸ßh°ÄÀ7ó¢²G‰À:¶³žþ]i?ñß°	´A@æˆ*?üùë`á—4¿ÞAPb#¿ÖNÏA­Z¨¿×`·-†Ô¿ÙÚX³5€AGNbll?îv`-9?¢†òˆT? ?œÑšìôÃ3?šTxî¢aI?"baÉô€E?'ٕ³&?íuýM?¾¶¾K2a?£—‹óo?­Þ¯AYc4?£q#"¬Ã¼?´ÞœZ5¢ñ?é¥Þçã²?°R½!'$Ú?³«N]<8n?¡]n9&d?¿%ÁZ¨Ã?¨Óï?à×#'à?¶ÞrIÞV?´¨«/¨?­7mèVd<?Ù'adR?¶h{OOË$?ï!]¦Võ?œ*)º²š§?"J¿¤—»?•pF*r?ƒI½Z?…-H'?îÅSR¯á?±Œçcàe?"Û%±é'B?¢À³IO ?'zx¼á9š?¥ŠÇoã	?ë¬J­jÔ?¨ÈňB\?®Í@¢û?Þò"1¥¿?³7q†+Þ?¢aPçt?撇]:ü?ªƒÔ;Š‹?¸@j.k$?Ÿ6ª¢Z§N?ɕ­u]i?¦'Öö‹%ýAGN3FGL J1445.0-0328@uÓ1ŸŒ¨@HuËCòžÀ9§ËtÝøÀ;p	{¸¿îÚœ"ê@,"+ž>o?ÿIØÿ5)Ø¿á,š¾ÃÛÉ¿Ù0õÿ~®d¿áºì¶)м¿ÖæÏ7—OAGNbll?ïîPŠSwï?Z–ï^´Î¤?O–P6O_?IÐ(õE?SÛ pº‡Ž?RÓÆ;8:Y?ïµÓ¡}=Ã?…ù¹k¦T?pZ#ÀÚR?þ>xM|?t¼™D>Þ?wmp©ßڕ?ïÁEÇy?‡kMɼ?†öT%^BÝ?xVÂö‡?'̤	¿Yb?r B'®?ïZF@+>?…`'û/@?D[6¥¸º?C¨—BÅÙ?"]ƒ¾»è?….oo0à?ïúëæîa?:8€ÓĜ?2«;×q%?,ßEªU?5õ§ú?2nVô¨8ç?ïãþúòO?sÔô]eY?ZǭΎԩ?pÚ^ˆ/º?]:\6Ն²?[ʐQÝE}?ïšE¦J`?s'ŒºÏþg?v¿LÜ$¢-?f^èÀ3¼d?|.áä9è?mñ#I€Z?ïÙ¯éè ?bý—9Ö?# wû,s?åªçÝÖ?r‹VÉÇ?aÞEüQµUAGN3FGL J1446.1-1628@u,ù jn3@C$CÀI0ËÀ9á·äkOÀ;†­âü¹ú¿ìùËVÒ@¾…Mi@ßy_'a¿èA5Ø)!¿ã†È1:=F¿âÛåÍ¿æªÔͦ^AGNbll?マw¬´Ô?}н⅐?T‹!ãF?M\Æw¼Óê?{•ƒþ.q?|el*Ê}Ã?ï…ÏtiV?'ûŸ»ý?z§
Òy²?'féEŒÒ»?jÀ­J¡?ˆ´ùÖÌÿ?î};
-vA?'1
¨¯î?Å'?s®/?|ò¥!±,?Ÿ"w•W®?ˆ¾[òyl™?î²ÝZc£¾?'DÁf$D?j¿ï9\Ê?fÆPBÍÙâ?£&+bÚ?Ò?»±Õ!Ez?ïñ5ôrqü?ZYån@9Ö?<¸‡Ä+?3ÏpüV?Veõ‹SÐ?WãYI?ï׌ž´`š?p=ÿ v?a£ [22?X–œC×î?fÐ_ÇSª?kN¥pb¡´?ït.>hÖ?t—"÷m†(?|C\s
ö?aж9Ð?"ÒÂ$ë+d?oª¥§; ?ï²'ÙÃ?p«Þ‡3·O?I±›_-,º?<á§¯
?ä"4ûbÌ?pXª½¸š¬AGN3FGL J1446.6-4701@t(Óõ¶@&ÓÈß'·À9äþú2À;]Ê÷àvÎ?ïû¶' µ@xߥA˜|@bÏߦÄ%¿ê Ð]â¡¿Ô+ÿÊrvâ¿äg=› ¿ïþ¤&Kª_PSRPSR@?ã™l'ûDÚ?Éöà %ºO?Ø#V_ã€?ÉÔ¡UXT³?…:p`eE?ƒë«Ç¸{?Òò\7}3¡?ÇuÏ`·+?Þð¯âӖ¸?ȓÛ×#4Z?Ì9çÉ8©Ñ?ÄJ½Ø,L?åqZõ¦?³†b
">?Ðuž)?±°mÔ®hj?²¡%†bµK?š±6?î\³?ÚÊW2}	?·qRZÜ=°?ܸ(këÔ?¼Ò߃Ö?ÀûÃ/¦G?©âo?ê?édֈ&C?Ã53*FG?Éäù|µ?Âò'*gæ!?uPõÈ7÷q?u'ŸÒ?á;ٝ?Áa?Ȭž5¿€?Ô^§å%¢ì?Ä]];¢öî?ÂSIÀµ´¥?½yóîÇô?é˜5òß?®¯ z°?Äb€äÓ?ªá²ÔQq$?¦•‰%Ä?"m×4L?æÈÝ»¡E#?¨Áé‹G¼ð?ÌrÎ$vèü?ª$AëÂ7F?°ÓuØP6ð?—Á!֑)MIXED3FGL J1446.8-1831@u••:@B:)@k*À:q?8$4À;›Ÿç't1?ãU4%‡µ'@
¯–§w?û'#¾Ì#?߬$Éì{F¿ï'Hˇ
·?î¦ïc"¿Ó±²ÚÞ2{AGNbcu?ïë°¥yÌ ?eϒä•?0"81Šy@?0s§‹Èژ?b<ÓeXL…?eg¥Ë×?ï'çŽD&?q(2å`?|u°ÍÚ?')hO8é?@¹hƒ®?‡Æ'ºÆÿ?îà»Zù?"à0-¤ß?…Ë_ÉÆ~?xÍÂyS?¢{™ÿE?'`9´SD¦?ì•;ËG?ÀC²<'Î{?g>Uvº&™?'nŒ*"M?ºœ4‡#ÓÍ?À;Þ䍙í?ïôÓ½":?Wº:$ÉJþ?&†¬—?%[VRfq?S‡¯¸€?V÷h݇*¼?ïÊç'þ?"ˆLrÒãñ?i•>qæ!?píæK›®?kƒ™èG÷@?{Iqº_¾S?ïWëàt†?Œ®péEU?~š"…‰?xî6ðP6Y?•.z¢ï"ß?Šx"õzi?ï8H¨j?œ­¸p°}r?{¾Mòhö?…6Ï$3ô¡?'\M…ZM?—v°™7
AGN3FGL J1448.0+3608@N"ˆ?Õ%@OÛ¿[o'À8߉çtî¿À;;Ɨ(¦?Ø9scÏÞ$@×vôÓý?ý%ßbц¿Öã"8'þf¿Ùïw`x‡¿ÙAúÚ.è©¿ÕñÆOÖAGNbll?ïüá?J˜«?68ɛ¥"?$#ï'5Ä?)3ˆL'Õß?-ÈÒäQð?+Ï.Ôç;ü?ïµdðç֋?ƒ0d±6l™?n¯¤E㚵?s
¤W\Ž?uõµˆ¿U?}²'7õ?«?ïV,JÇà?"e '¯r?''˲۳ê?wégǖUb?ˆM!"E?€W¦)¥?ïZĂâ"?ŒtöEx?b°êƒjýÖ?`uÜ£¡Â?›^Šn½Å?‹ÿ¡•?ïþp6&‹8?$w+ÿý?bÑX«‹Ð?¬·Í³?–dœëëA?OÂBÉ6?ï掾/ŒF?fÇPF¡r?VÝ[Î?UêçÅB?\/Ý֜?_l7Ó{?ïžaĸx¤?|Œ%¦?wxÄÉ[q?p¥@³?y³¤ïxrQ?uRO\3?ïÁ•^ÿóH?iG'Cďä?UAŜլÑ?C
@¯«
?yäßAÌ¡?h/}$"´AGN3FGL J1450.4+0911@ lŸædÎ@LUÁ HàDÀ9íþu¼D¿À;»˜õ.릿éFïþ€#@
Ç+Î@ʽ`s2R¿æ°²ë$P¿ßt ×·¢¿Þ}®±Ù¬Y¿ì6ʸ(-¤AGNfsrq?ïªH;`±Ï?†Dÿ\F?ƒÆK"V b?…á¹o­ø?JzX¥
ԍ?Hä$	þA?癩*XKÏ?…±ÑBhµ?sG¿7ˆ	~?rÔx_†§?zq+"DË?€†¾!ŖÝ?î÷íj"·?ºtwτ?¥SA§‡qc?™Z9kãQ>?•:~û	€o?†zü¯ðFo?ï'Ra³?€¦îOT*<?a¦))Wé?_°Õ'å–?‡S®›"ä?…ŇJ?÷?ïÌ®˜?›?vÜ» _Ãu?wÕøé5C?v+ݖÛœ?=+®tx°¤?=Öi¿MCn?ïߦP·'Ÿ?kÔh¥˜?]ŒÎz?Wudu, ?aÓhÚÎYø?cúxѪÜ}?î«KǘtD?–±Èf@
Ó?ŸAֻ͋Î?"Xõý³û?†©rñkd?€x#Ù .,?ïé³wž?_:m®is?AÒá ¾?9©Bðgï9?b£Ø!í£ ?]‡KáÇZAGN3FGL J1450.9+5200@VGŸõÔ-@LF{ÓöÀ9Á
Ìq]:À;¿bÀ¿xP?ða#""@7_a@k=ŸrÌ{?ïåq Ã^¿æ>Ölá¿à.Έ°=¿èŒÚWéÀAGNbll?î74SæÿJ?®ÂZé;µ'?bUêÖÀ?§R¯±PH?›·˜Jò?œ)_ç	?çÐw;BB½?Å㫇>Š?È7cUKÙ?ÛˆÃCÈ?±
€gkf?¯%_üî<?ë>'\;?F?ªé¨ûŒRß?µI˜gõ#?£"M=[¼P?°ÂT·õ÷ª?ž
€ÂœÃ?àæ»ãñVš?¼ÇG':Ք?ÖHsb'?¿½F>u(?¿©Üv§Àé?³p €Wm?ï
œÊŒ¼Î?²<¸ïª…@?"÷‡ Ä	?±˜±.?…i¾âԞ?"–Šº»Q?ì3Վ"©3?»ŽùÏܙ?¶"\m|Ú?·i!µ¨'?Ÿ3܊áÄ ?£³H¥ön?íôãiœPÙ?›ÒÎ.ü¶­?£‹‰?"|'ZÞ??›5v¯^ÒÉ?Š÷BîÇ[d?éVŸ"¸çÆ?°,eš=ÍN?Æb,z²MÆ?«] Qæý?¡
TÇ—‹?šÂ*8a(AGN3FGL J1451.2+6355@Yæœýç!@H;ô|ôÀ:ÌVô›¼À<,SÐa¬Ã?Ï+$]¤Ã;@ÿ˜_ݶ)?þ°Á(~Ï¿í‡t[¥ ¿ÅíF挎¿ä¶ˆî¦'¿ÎùƒÆëÙ¥AGNbll?î¢H¬c˜"?«žË)+÷?ö.ÉUĺ?šÚ·ñôNœ?šÀ»¦Ç›?¤/î·Ü]?ï}¶ÈG ?—ߌ •iè?€•¼rž?6GÆ°V‰?ù#×
å?†!®Súy?í+'#†ö\?£Å Ïç?¢¦F^àÀ]?™÷ŸM&",?ª §i‹ÀÛ?¢)ÀWn\ò?ï+ÑQÒí?'îÖ|lñ?‡•é†¢ä?Š`¡ÿZ?©b	(¾?†ÂsÌcB?%x>?­+4"µ™?x»±ˆÙò?¥*Äøã™'?'ИÉæïˆ?˜nÚ~;DO?ïÛïè°®?rÓ+ô$'?b›f:-?hh
«õFÖ?b[©´òÎ?d ž+Ø°?î'röš
?˜11Xñ'?˜J³—"ˆ?"/Mãr1Ÿ?•†í£Àì?ŒÈ^þèþ²?ïÙèCNH?iqÀ®¦²	?eNÄB'ì?`QåÕ¤86?`Èø"D•?\ëFo°þïAGN3FGL J1454.0+1622@2Œqà,l@MÖû¿ÿ^ðÀ9øNz·VCÀ;ÊmÍÓ?¢]‰3ue@@ם¶3Ù@¿‰ÿ¯~¿ä!¶"F摿螓è:ø‹¿äNþC^Ç¿ïÿïÛ*ï©AGNfsrq?™è¸ª?¬I¥ØšŸú?…o-èµ?7Šü6? J{ò=é?¨«A¸ŒAû?î±(Oo?Ö¸ü
ì£?—t&Å–?'x®]8#å?'ht7Ô:|?'ûJ:kÌ?ëVëxxP?®ûšÀ‹ ?­Üœpàÿ?žÅwj†
å?¶ZVñ?«/=uÐhm?í3_5ùÛ?¢Y.7©m*?¨^Ô
î1?› 'ÃLׅ?¤k8'¤ª/?™dÕb_«?ïCXؑڑ? ,!ˆEFL?"‡¼†àWº?"Fàô}ê?Š¢
T©?–/)¹6íÓ?ï›ZûèÝé?"ÓN?|À…±Ò?é?uo¦Wqô?u'üZn·t?q§~çk#"?ìË'´^?§–d/?ª$8Såw—? ÃÒäO1?©*6§'?¡='Q#j?ï[a|¼i?Åë´Ôëx?ˆ™°Ì®Ge?t6ÜL3m?€Ž©àH?uòSþZ'‹AGN3FGL J1454.2-3751@t'Ž wm@2ìïÔ;VÀ9R¤ÅFƎÀ;qÆ:âT¿ò7wÀÖÊR@ks]oǹ@ Û´¿ç6üºavy¿è×{È´uy¿îs€Wÿ}¿ÉYSæ(ŠÛAGNfsrq?ï㕶,™³?oM%Ò_Ñ?bÖ͊ï~?kq	ž"?S&ø–lüø?TùgÎ:Ì?ïš
ä³ã?õ1}£W?oÛgx°þ?pðæhÝ?…¾÷qC?Š˜ð»å*?î;&ES?'A¾Œ#V ?'</»lm¶?â²Ã­.?žœl¦ªå?ŒÎ4Â.­?ï/g›½Ë?'ºU'#Â?EšCìµ?Q+ZÖ, ?™f:u‹f?'¬°!ÆNX?ïôXC&à?ZÂW§&?N
˜w®?V­®ºk2í?@"[Ä>÷ß??ÄV˞?ïÜKV%â¤?kj®7Ån?Yn´JÃEV?R_ä!>Gp?fýO¦ýIˆ?f€±ofþ±?ïPô#JTY?ƒARk>à¹?ƒH…Ù‰ü?y)§BHÄ?ˆ®®°€[?yÂ(en(±?ïÞÆéwÂ?f$µWÂ_
?úMq7í?
Ÿ<3Ã?p^–´I?fOµÐRAGN3FGL J1454.5+5124@Uêx $Î@L9o¿«|À8W!CF¦­À;IŸß-øa?ð¶zӅΌ@»W";Œ@«¯‰øè¿ße5x÷|¿âBÿ÷æ¿áï'Á;§ª¿áì6CmAGNbll?ïü:¡øžô?7™¹¥1•ë?,[[AôÍN?*Ÿ\­o+?/úƒET7"?+6ñ5êð?ïrf*ñ	1?óóDjD?€ùøb%†Ç?†:«µâ?'l|Ø©1
?‡\ö°]ñÇ?ï*ÛâÙx?Kx;Šw?†K|(/?~Ü}sc?Žý‹(	*î?…vÕà¡ßÇ?í]ñ§"g?¥6Ý ò8?›Ïš'K-?'G&°:?¬9}äØ?£x|Ì?š?ïþ	»ô?%×È£À¥ð?!é[žu?¯¥—v?õÒ{¶Ü?Sm´¨ê?ïÆ74¨0ê?x§6pðz?kdhM.ü?f· Õþ:?nIf±¨ï¤?sR‰
½_¨?ïƒBh

7?
J,}CC?€#Ï+Ž†'?zI‡7¶2~?~-«KS)?q¿¿0¡x?ï/LðYÕð?…hÁôýN'?‹—WÊí$?t÷EiPo?ˆŸ,•/2»?Ú¬ ½¾RAGN3FGL J1457.4-3539@tž5 ÝD@4‰4ŸCý†À7he²â?üÀ:ç·I­Èü?úMÔ§6»(@D}Ä&
+@\'eîqb¿à
´5Òñ¿å'Úák
¿äã\C«Y¿è'Ÿ5ÁOAGNFSRQ?ïÝãKµ-?rb	Õ¬È]?dk"_k"?nÇÁ~?[bÀ˜ü°©?bð•¢¼à?﹆@÷A?4"Âù?l?áG"?néaÿ¶›h?u´%»?zWjs³ûH?î³ñm&ZC?—À֊ÀØ?"Ñ{ö*.?Žª8Î'À¹?•°Vj2k?Ôt2˜2Û?ïðdö
?g؋z"­?ìW#ÕÕÒ?*äøè÷g?]ÇNƒ|¾ñ?g¸¢Î?ïçSš)?v5ƒoãŸ?bØbÄ{³•?tá™Å.äí?H=%j(?\‰NɎi?ïà+¯+?vì¡í½À?[°Èšn?mžãÓË?bM$õ҅l?jäÙ[ïöŽ?îÖ{H©?—U¤xúûz?–•66	?'~±ÍFë?6Ál£?«?‹®)O'êÄ?ïý 3žŠg?C€…én¹é?>¥ù?A9þ•‰?4à
»Æ?C0]CAGN3FGL J1458.7+3719@Në<¿£ï^@N°q?Þ<aÀ: –Ϻ¾À<DðÊØ׿È$=Æxä‡@¨ÜRPÚ¹@êvjG¿äé¯z<Ã;¿äiÏ°""¿çñԇðé¿Ûœ–½àåwAGNbll?ïê"!¸êö?`'L›í?E`§_R
?E›n#™-™?`´Æq·?\
¶À˜¥?ïµ$ªâÊÄ?€Ÿ÷¸¥ü¾?p"x¬Û\?q'-F¯CÔ?té1Ø ZA?wY:ëûœ‡?îÆfA[º?sg*Üw?®ûºýÁ?€Eåj¹¶?—ˆÕqÏ
?'IÏû€?ïl	6>O?…샰Õô‰?o	ùƒÝU?n9µ]p¥?;4É;?"™:©î?ïø÷·uçR?FUê.3?1ïu/þ ø?/2/©3{?C)h_¥qu?Ba4=,ËD?ï៑D$a?háq{ÜÚ?\ʙ'«e?]+`5Ó©?_öD	Û#9?_-"p¬±?ï|ÒÍS¸?vV}?~ìÓç,W?pŒ
™n†?Tã g#ß?c­¢†Z?ïè†Ñ×ë?`YÜ;<›?NI3ñŽ>?A³E-Or?_ÍÃÃëû?\V‰¡g_AGN3FGL J1459.4-6053@sÞ
?‰'Ë¿üƌ µ,GÀ6íF4—·AÀ9ûÏÑdB@hzn±@
E\-}@¥€
¿Ý¹›¿änì
Än¿çÿP§Ë¿î¶œxŠðPSRPSR?Oý2A]?úÝÛxén?íPšÆ¯F?¹š†Þ{\?µu•Éaz?¹—'ÛÎâ?(Úoó͐%?WUñͯð!?ë\7¹TË?¶¾§_ÉÌå?ÃÜXƒØDÙ?¶ nŽTÌH?Žo]qOlˆ?"²…EF'¤?è®7‹æa?¶A†'än?Ë`+ø	7?µsŠH¨AP?W›ëÇy|Ê?T _'"Ç«?꾍tGO ?±ÿM"®Ë?Ä֒WtÊÇ?±ï"(!h?8K¿y?ù{öà?ë?'‡]?Å3tø¿3?Áɾ:ì"?Å2*óQN…?.QvÊ.?ö?KbùBØÎ?ê¥ØðØ«ä?³–¨ûÈ?ÅaÞ,ö?³X^ P@?'øš}fª{?Žyh± G>?éhÅïÁw?²í€vˆ?ÉOI˜"$Ô?±/_Kçu?_#ÀX.?UªäÊ	n?ê•ÀýÇÒ£?ª†ºáFa?ÅjÃÁ
×?ªœëVPSR3FGL J1500.6+4750@TGŽÿâ£Ï@L¸®Ú«³À9þÁqN÷µÀ;t7.jv–¿çVjòß}v@ }kœÆ@$ q¿ëŒ$œJ+¦¿ßL©_Fë¿éù"€­ºc¿åø"–ðAGNbll?ïî|~+?f2+€GGA?^°à/È?eße½‰b?4˕í?3Lè9Hê"?Z~s?Š`½wGɾ?v¥d64N?x–JÒH/?|n"]«?'CuÎøÆÝ?îtÏc'0%?'ùô'x¢¦?–Su»‰?‰NÅÜÑ?›×åÜH?†¹e)£³?îh•©Ù`?˜.{rÏñ¾?'uo6ÒK¨?}-t¤
?¤ÙS
AŒ?•Ê#BM£?ïú¿Ö3È?DZú/äÚu?>£{.j?A)yÞ¤ñù?'ÇRo47?'Ú+Øês?ïÝ'Å/¹E?p° &¿?_tûîæ	¯?_Ýw^@0&?c¼ü¦?e­Ã4¯€?ïJҘ'‡?"ñðþÏ;?†'ã"ÙŸí?}jՑºxœ?†¹vWüÌ?zÅMÙP	?ï©Ŋý?sã"þ m?Zœß^žÀ¦?PRP¤Ø­‹?'h0xhP‡?r´£ñAbTAGN3FGL J1500.9+2238@?pc_Jé2@N.µÀ@ÍPÀ8î÷Œ"÷™À;N;õy"A¿åŠ<ïÊ}½@é×µM?þ±J b5ª¿à'Ì!ÅçD¿Øz"ZóÁƒ¿àørOu¿ÕÓËÕzWAGNbll?ïýyÃ9Ú?>2Õþ¿?ì>Að?)£/¯&¤Ž?,Xü;"q?7žÅ}fŽ=?ï¿þèÓ¾"?~ÑOû'M;?kÌîم£‰?qôO¿þ)³?r%>d}?t…4·1¥?ïY?€׌?"M•áŠ¬?Ü~¹vN?}bþ|ó¿?‡Ó¡FD¦?{f/lþ¨¶?ïÊqY½?rݸ+yÜ2?»½	Ó?!«_=Qs?zvØW".\?rÅRd¦·?ïú
|ÓÅ?€./-äž? žJ'n0ý?LJååWG?C®zϑ´Ô?ÿ)ŸvO?ïèQÐ 6?g&%`'*)?T›Hxó9|?SC;"ÿѲ?Zª
Gúµ?aC"t‹ '?ïž|Šj&º?~Όsvd?vԗS' ?ußõ\"®…?yí#"禕?uÛÊË{£?ïõîÓÄ?QFÿ0]Ô?·5[g"->û@Ãð68¿?UXBù-4¸?Q;oOí ÑAGN3FGL J1503.7+4759@T;[À6ã@LvÊàc'†À9ƀÈè;¾À;›)гâ¿Ø¶á´'@ç÷ˆã@½è@EÀT¿Úªüg´¿å>¶DRÈØ¿ä—$äæÊ¿åŸGïêAGNbll?ïóDf³?dԝ–ù?HÇr®Éë?dhš.{#É?J&õdu2›?B˜rB)øÇ?ï±ã¾g?€R–,×m?q#ÒMÛL7?p(%7mè?uêNiü½:?y;šR)­?ïP…Ço?bjˆK?€i¿:€Âþ?q¸ˆ$%…?‹"úض«q?x»îX6?ï¨>šfë?Œz´$ÿ#?o–'ŒçÒà?dZX1¹›?šx%øÚi:?‹¥'°è;?ïú0®Q?@?L(ï1hà?:!×'
ç?J=îÖÊGÛ?4X´8ž??/.OÎwíí?ïâéDZU•?hD춧'p?Y´H¹X®ô?UÜvö?`<—elP?b/ñøéÕÙ?ﰖ˜³?³?pO/?pa?;E?`»Ú¥•2Ò?wSt	ÔÍr?k*S´\¼b?ïÎ(îûdª?j햸?Q¨}K~?@>å׌?tªžS,—Í?iyRxßAGN3FGL J1503.7-6426@sɛ€#¦ÎÀ–šÀ
F«À8å¢4rÎÀ;vJßø#?Û毶UUâ@­êY$´j@¦¬ l¿àjÞ|ô|¿ç«
ü÷ü•¿âÄjMÚ1¿éEpÑ4¡®AGNbcu?ïµóïó»?}¦Ü
_¡•?jEËNèq?o"Øe?xS |¿?vjLŠ'LÔ?ê"åëV?ÂÿO'
? †^e|`Ã?¡îSê]¸?ÁŽLÒt48?À!=kµŸ?í}L.VÕz?ž²™ß~o?!Ú×b¹?ŽmK:™?©šO¯½2Ö?–jÎkb™?êT~ñ¼_0?¢N(%p?"LqÊR#?Û£fæ?ÄDuÿû<;?¡ÞqĹ9?ïä¡ln4³?gýó'e?Y÷Ìç?ZÌÁY?]¡/\.j$?\ŒüïQ¡{?î[ ?Ä?¯¾"ðÌ"±?ŒûJ‰r!?ŠÁzÂ?¨7O'©"í?ªwÏÈÜ?ï!4üi¦?‰	êŒÊ?‰
¶";-?€;¿ë¶?Ž•¯@"E?R›bWr2?îí%˜üø?‡òðð:?†áŸÎ¯(Œ?l5³õŸ,?©èų M_?…`S§mAGN3FGL J1503.7-1540@u|0¸,,@B?ñ7À9&M±cººÀ;*"ž­Õ'Àý¸à[Ê×@¡nu©z?üPOÞº‹¿àü᫽CÔ¿æóEkˆÓè?©Ÿº"®´<¿Îs0õÒeÏAGNbll?ïïnoÊ=P?[ÍyïÔêv?5ϐ!¦èê?2,êÁ©c'?[¯<dµY?ZMÉ찈m?ï»aM€o?€0nãݒq?kUBO¤c½?kÁöÁÓ™?t¤¸–t=?wÆI£&©?î´4§kX?'ïA#³NÒ?‰gŽ­Íñ?}åö­?œËò2r?† Òú·Œ?ïѩًT»?z]|3·zq>¡Èùö‹½b>º–MY´í?w*"ÜõÄ%?z]I‰šHÅ?ïùOv­'ã?CN¶;
e?1¡#Öwk¼?*\ç÷•¯j?Añ"ªé	†?@5dL½?ïäýöew~?k9ç«>?U¯/û"º#?Tfécql'?`*q¤ý4Ò?eý¶Ç?ïc¦°Xx?'¼Àà6?|–V-0'L?n5ÓªD?ˆïkCX?gÞÄò'ñ?ïöC ´?T#{Hw>užF²'‡>†éÜ$¡CM?Sy‹"@¼Ð?Tîņa¢AGN3FGL J1504.4+1029@&Û`C6¶@KJ0 Y;ÛÀ6"bÕ¸-ÙÀ:¨
ހ@ÀY#²·£@"så!Wh@;l0ªÂ·¿àŽ™ë4¿äˆpeSýê¿åRԐæl±¿éDŸ¶š©AGNFSRQ?ïÓ+Ý×®?v%)@$b'?foYuƒb?r_諹ú?fe¡}ê?½?eÍD@Ÿ û?ïƑ涜£?J°&ÀN?i²ñ/àÊ?p™ëƒ5å?p*³7ÈiÌ?s¬·,IX'?ê)3vÂ?±÷p¤jÉq?»0Ýû?É;?«O']ø?³……›4ú3?£…ü¤míu?ïûpےì?a:P™ýð>ëp–ÇÈP°?#ežùÝ?C€y¥Æî"?a6D¢SÌæ?ï¾½8–Z±?©i˜-µz3?UpqeF£w?e…$…?{EGx]¶t?©fͺ>œ÷?ïæj@QŽ?j®k®õ?V€N'?mY¶±"9?\«1KsÉ?qÓþ¨''?êç&ò!þ?°Ó'Ùæù?¸P]
Íô?©"JFÂ~?°vka	ö?¢ÞàºYF‡?ïÿsðN?(¿´íOQ¶>áçs)º÷?²Ø—ÞL?Š-ÿE5¸?&ý'Ø·3ýAGN3FGL J1504.5-8242@s3Y'ÿÀ4øc ¹HŒÀ:WG6wÀ;·^j¢Ž¿èìãuÃ@Í)éÞV@aÿ ^¯¹¿é³· s[¿åqµ%ªù,¿äÄÖô~E¿å/Ë6õŠ†AGNbcu?ï×4§§yV?pTÖÌ°?MÛ p
›?Ní¼©?pªH싗?m²€^àr?ï,}ÖM2?œåùª·ŠW?t­6B¢a?s3áÔ§ÔÉ?•SÂÀq".?š'‡˜àî	?îNGv¿­ˆ?"1-+õ?"½Q™J T?'éK>ÿ?¡<ßÈ;¾S?Š…ïŽZÛ ?îÁ5P*  ?Ž2h•Â}?\§–½µB?V5ïBpýi?£¿?Ô?@UÒ?ïóŒ®hw|?P~.¯löî?5#iõÝ?36dREU?SÈÐÛN—?L¦;ÿÝØõ?ïÁr)y\I?|!'ÖoÎp?_œhšÿ"?d@'bǁÔ?w_Ñ23ó?vss²p%?ï_@'Yrý?v¨êO€¥?4·Òr³¼?oROô+*ç?†û#ܯí?hÝÞ©)jÄ?ïÀM?w©?gÔë¥c%?@ÃKî	2?2¡ö?}Á'¾†š?gC3÷ÍXAGN3FGL J1505.0-3432@t¾¬à2Û@4³	¿œb¢À9­&|k‹iÀ;ÞŽ–0Y?ᜏ Ï÷@ ƒ™:@×ýFKê¿èäÜJÚ$*Œ¡—¿ä?[ ˜D
¿ä]cMWKÁAGNbll?ïÇôùð$?{Ü
¶öúX?vרe<ÚL?z[å	Sæ?T·jl‡Ì?PfÙ9'û?ï"þá-=?£¯­y—½ï?ˆÉ<(ã¯?‰
~ü,¤?¨âHx? lõ?À[ç?î¾À³—?'ùk§ž?'º¤OVߞ?""S}'A ?•ƒkCz?¾7a@ç?ìÛM-°<s?
8¯ºy? lˆt›Aì?9%R¯VC?°ïRV
¹ò?—ªz-Ûû?ïò€ vÃ?^e|‡>;
?V'ZìAՋ?\vÞÖ%W?5F"õ¯0è?1¢'ƒ‡?﯎J¥?‡¯0gxu?q¹¢$¸à?lì,¢Äb?vÝÙVh?'"-ìÀU?ï€Ì»|dÍ?zÆLÍ'°?šÜ8eÁ?sy&;å½?þÆÄ7à?l÷lyι?ï˜Íäj?~I¯qtó?ØrwÀ?nCÂ_=?€Ú
AT?x6þ'ÉßAGN3FGL J1505.1+0326@ä×?Âb¼@I ÷þ½áÀ8…,$K9À;p§I……?Ò	®³@4؉™q@ßú D®†¿å6}âÑ=¿éÿHÂ^¿è иØ$¿æI̧¸ìAGNnlsy1?ïÅ\äî'Ö?z<IãÊÿf?nJýk‹ù?n;` ¡4?lXÿ2>-p?p'!:5þŽ?í´0/|^?µ¿—
°ê/?¥ä:HÒ­?¯àéí?±yÚîjÛ?§DW°±‡N?í^ÓR«|?£«¡ª›ZË?å<*U?'_1½?°Â´t?ž‹u-meM?æúÿ›Ý?ºXÛ?ÀÜ@¨f»÷?²'¡—óYÝ?Ã7Ãý?´/móüÑ?ïïf‰ï$?_x#!),?Qc¨Çæ?Q›ãø¬2?Oǟ;'F?SÙ=ۋ·?ïG-qZé¹?¡všZžh?Š¢ã­)'w?˜Æ^Ù=¢?ƒ'¿þ+Ã>?Ž¶	õƖ?îÁG¢ßq?"Ì·r*fq?'j¶µ¼Ãs?‡²ÀñÏi?–r`Rw²n?‹ s˜ø
È?íé%õ,p?˜Û"["D¥?‹§ÿ¾Á?ˆ¨5eRð1?¢§ÚM^š¥?"›WãäAGN3FGL J1506.1+3728@NÉÍ_™Ã‹@Mò•¿ðExÀ9C×xø9À;É}»Ûä?ò]§rö@"äÀ`Ù@Ÿ+À£Ò¿áõpÙ˧£¿æ.5Lèæß¿è«øP€˜c¿ïü8—Ô¦AGNfsrq?ïí lq˜I?X÷ƒ;ך"?Y0ÍýRn?SC8–Èý?G±Ì~µ?Eús'À]?îº6 ?§= ‰ò¹o?¤nùn&µ?¡Î–b˜Öš?—%Û9±?•}E%#%?î^Ðap¢?–BH*åQ–?¡ý
ŠÁµ?'~ٞ?'çù¿m?~?…Z´bð?뼨+n]?­ß$?ÀÙ?ºÎs.æ?©©…6^'?ž6¹Yæ@à?œÈ˜¿ç҆?ïòá2y=È?Tq¶ÓŸ?Ubûå΂X?R_² -ÜÚ?3j}
ä­?,Heý?ï'ˆ(hÌ?'b¹ÚÕð?';6q]
Ã?‰ù+}ñÃ2?ƒ§ŽÆu#|?~œ¿k Äÿ?îîÚGx~[?‰«²pŠ?—@)ûKò9?"ÔjSoŽ?…É<vÇ?rS@°Ó~¹?îì=¬øŠÚ?ŒìÎ÷~º?W#ÂÓk?†H­TÈõ?t"šwó©?{^U4œ3AGN3FGL J1506.3+4332@R>Dàá6@M#˜ÀUÆÀ:ŒÅ½äÒ}À;ý¬Y¾O?ËV‰?•}f@
Òæ6«7Ò?ÿ'T€	û?ïð·EçÒ¿Ï"ÑžâH¿Þˆž«Ò+¿â)˜'©AGNbll?ïëW5OÇ?d•ÑȽÿ?G˚Ùn˂?N€¿uƒ'?]kÈÝ Já?_'-ƀ»#?ï9b†KÍÎ?šÀ6]×n?Šd/m‡Á?"bS!ß%?‡CS,pøñ?Ž'SâóX;?îìR³£}k?†äKŸÜ+?"cØ>0l?~Eù-ÕÅ?"«÷¨@m?~Žfôw~ñ?í3ø»:??§Žèüoq?¥GáßFc?›TñŒ?§x'qˆã§?¢3‰á'Ì?ïçÚyd+?‡ŒZ·×S?I{ђC`ë?iZò‹Zà?aÆñ@÷xf?ß¶CQn?ïÇÀã¬Ú‹?i5µƒÙä?l8ÓX®?vV££ÿ;C?lI8ä¾'?n¡?fƒ}à?ïuÕ±;»‡?y"€ó¯_?©Wßj÷?rÖ2"5L?'µçħÏ?o~Ñ®<Jª?ïyCù®œ?£ÅX˜4?ƒ¦7ØK•‡?pÁqÎ@'?|Ï5´Ï?vƒIø¦Ø7AGN3FGL J1506.6+0811@!VèË@JiÙÁfgÀ9µ/V/À;€«rßñm?ëNÜ~h@;=‰ù=™?ýûö€¥Vç?ÅUw…úù¿àŸKã`놿Ϯ"ý¾¿àÿ{τ7AGNbll?ïëHø¹²
?Yìˆg4È?YšçGXv?R¡rN…V?P^t'åº>?Gf2pùn?ïHo‡™´>?"6Óeh¹?"àM¶€Õß?'3ÃÃc†?‰ÐUSª³?gQЭ?î؎ر˜¥?'Öým͏ ?"®?‡Äë?Šœc{äøŸ??åjŸÓg?~fZæ:½?ì"É
Aï±?¦ºuL×K? íb|{Õ?œß}Ã>?¶s£V]?¢¤ø
ìrr?ïòĬ~	?OP8.°¬?Pj—ö½?G<"zM?D!×¾Ø?<\wh‹ÉC?ïÁ"r1Ô?|¤"¢"‰?oµ£¡>ƒ?lWɄ´«Q?og=èÍ=?tdåYøé?ïpKÁæŒ?~F?
^ÈÅ?"…@)!?w*ÿŒÝ?~ÐE$9×¥?hMþnè‰?îw›
ï?†2
I?›™U‹"«?‡'{Ò°Ó?•…ׇö4ù?'=ûP¸AGN3FGL J1507.4+1725@6ëòÿf}
@L—«ßí;À:—'ï2RcÀ;Ñ<*R¹á?áËÌVÛ.@«¤íµ¥"?ü‰!ACAH¿ïê(¯k?ïšÐsÓê׿Òî0÷wN¿Ób¡éAGNbll?ïý+—Cº?-ÇäÉ¿÷ð?'E·lì`¤?"'Í`&É?'w'£(S#?"F7´awÅ?ï¢ÒÒ97?…—£iH?v(þÛà?zÑ+§³Ä?xm˜Ï7<Û?|¡|F…_?ïk¦ž(¹K?}l0ëh?ä'ÄÍ?q&ZRËðª?…Œæf¡?sÑè;ô¾?ïVþ
ÿ¯Å?‹gj\+‰?‰$€˜	ÚF?"ñ‡<*ðÈ?ü Óf?€¶À°,­±?ïþ@ƪÚñ? švG <?3&WûÖ?Ý÷|ü?´Œû{¯?_r2Û
?ïàùúu?fÈ-ú»Ò¼?]ZqÐ!Ì÷?Y'\ñ_½?`YÃÿ=t??_6PÅá:?ïªÂ¥›Ia?nŠ\d+…?s°·IV*ò?gîù鬩±?víõÓ·»?aù¶
 ¾ß?ï˪
U‹?oþ·h}#?shÙÆwù'?hÎÌ$‡þú?["³³º?\G»ÀôNAGN3FGL J1507.6-3710@t®ÿÀ	oë@2-×,uªÀ:	JÅöï¶À;Ÿ{Òuð?Ì1kKÂ:@
«$õØ´¸@jßÇÑ:?ºWZ€Dl¿åH¡y·Ñé¿ÕT…ࡍ¿æ…ÛÊý¥ïAGNbcu?ï×8UÜÖZ?p
ºÞ(ºí?K€¾Œõ?IêÀ+?pó½kùªÔ?l¸îðúXÀ?î¼ç‡Á³r?¦ê`³(sØ?·"QŽ ?"Üõæ€åß?—«Š¶;‹¨? ¶ªd¯¤?îµCšDËr?‹֝Œìƒ?ŽAN\Œü[?y(¦l¢?š6åÿK?ƒPøm2B?ëÒ?Ær\?¢ô¶Œùµÿ?—Öúägg%?‹4(—?»xCŸÒ?¡	ôæv½?ïóV˜ÛQ?UvÖÍ_?7èd
å|W?9ŸFå"Þ?SX¶ã?Q>Åò?Þt?ï'x
`n]?"!
à°cÈ?vòø§é_ø?s*zÔ9Ú?ƒè€T÷š«?OÌyžZ?ïtSëî?tBԘ͆¦?~Ü Cá?hŒâ'–?ƒÍ½…[?h)"2}o?¥š"ý?"IcYVI?‹P"SÓ@ù?pÿ{Ü~un?šaz${Õ?€Ž\íËXÜAGN3FGL J1508.6+2709@D€"ð½@MÈ÷`MÉÀ:YÞ9ÛÀ;³¤ës¸¿ÐŽïnYÇ>@
2ôU¿?ûXt@Éп圏º•¿âj­…+Dõ¿ÅÌò—mx¿Îå}éÃ[AGNbll?ïñ{Åj¥2?TrÈM¤â?0¢Gé¹TJ?.D¡Æƒ\Ý?XßãF‹% ?RÇên* ?ï¹¹J§?5ÄúÎ?o,°Çtr?psßǍŠ"?s°Ð"?uŽÁÇ[®Ý?îóÚL"~?†ù¿ŸӒ?ˆ;6?yNF$H©þ?•fõî´G(?€ºÇ²HÌ~?ïaE4	q?‡h«ÿ¼}
?IWAbʕ}?S)o¾Û?"ŸzÎ
6?‡Ú9ƒ‡?ïúY}I׺?9²s^·:}?"15¥?Û^®ÈLÀ?B
ÆU={O?7:!š¢?ïæ'ï³+¼?e¯+5g³?W¦‰ý$o?Uw*7šÎ³?\	—ø8?[÷ ÷m?ï}_QÒ¹)?u0'²j!?{3¤e""?nC¬Žÿ
Ü?ƒY_nÜÌ?jÏNQ.–?ïÞ¼Fubá?`Á'M±ï"?A´Güǹ"?:'ïÝeqý?lÖ§™oþÅ?^5Ò6þu»AGN3FGL J1508.7-4956@tF7GMœ@†¿ë½ÔÀ8¥ïm
ÅVÀ:ô"Ýz™ú?ã;Rø¸@C4LbÚ@Ø!¿˜[׿çßsâ3¡¿é÷ž€f˿筕~g1¿èœpc•QAGNbcu?ïÁIý,č?~Z[`æÚ?Rbœ°
'?Sd¸™í…?zÂZCʅw?}(êUƒö?퓨øËò÷?·ÅcA°Þá?‹ä££ƒá?	u,yq
?¯ÌG¨ÌlŸ?´úy`"ž7?ìwùÌ4KŒ?¦''bs? ¿É"ý"?"B̆ÀsÚ?³àLÜQ¥?¡mïIW?é½ÝqÆÒô?¨ŽŒ›ƒ?›"ÔD
$?‹ñ·J¬?Ť/µ$dŽ?§ÁÇ°	Eð?ïìBò‡¶?gý¨•h?8èÊÒ$?9²iŽ¬Þ?`R£Ñ)ø}?f'¡M˜á?ï)'t±O:? 7}y5G¡?yG'`Có?~Ñ«†'?"}ÐÓQ'8?š­'ä''ô?îÒì'ŸÅò?'üÏXt3¤?‡á¾	Óò?}æ%oƒ•?™±›Å£Æ?õm.?íÃק‹
©?Ï?ŒÀ"Æ?ŒyÞú]?rÑ´Šƒ¤?¬¤
Êo¯£?Zj¸8IAGN3FGL J1509.4-5850@sÿ?á—_¿ãÄ&½ò·À6ÿ\£oqÀ9ê÷ãÑÌ@äª1xg@¶'ž?ý˕/&´?»Í}þ'¿ß!]
ÞK6¿äÀj4À벿옗A‹Ì¹PSRPSR?AŽ/8Ÿe?CÀØÌC?í?"û&ý?½=Ì0½?·²ç{'RO?½&œ¯3ñ?0"¤UÀìç?QËrXY×»?涱¥¡\?¼U1—ª½?ҏ·´rôû?¼TÇ,¤Î¬?}ªÜ×\?r',DÏæN?é%
Ýîˆ?¹v:G?ʃNoŠã…?¹+ýÄ°Vq?yý?ËbåŒ?r)õÇÂÌÄ?åôÌC¡%»?³ïÛÕi¯?Ó®ryo,´?³âû_Í¿?/`›ôq?5ßÇ
?íl§¤…l!?ÀÄ:"5¸?´‹œìˆ ?À¿ø{?8•îV'¤?V¥7Š˜cP?èǼAº5?´ Ô—ä'#?π–ìÇ$?´¡±õhÉÙ?ytöp‹4?{=\sÄD?éúåC¢R?²¦3ëU?ÇLW'¯ž?²<Æw ²x?|"Zª?uôM±B?çGFÌ©L¦?­jXþϋ?Ðÿ úÿî–?­'¾0Œ@¿PSR3FGL J1509.7+5556@Võ: !Þw@Jߥ¥À9ðE;ss•À;ÉZÆõó7¿¡›÷êH7ñ@¬‹ä¥0§?ýí2?î,™¿Ó»6.\¬ ¿ß&ŸêŸ#O¿ÙÌ4mè2P¿ÏÞÇ}À AGNbll?ïüõ3̸?/Xva?É°ŸÜà?¡?ÿXƒr?0ãùùÃx?'Þ{Ùa
?ï¶5&†D?‡ÄϜB½Ö?pìÛ!ܙ(?'+Èdl	?sø'»m˜¤?ykPT-?ï'À¦t°?wˆÙÉ°?y5f3¦?qøDe°Â?~
»ÐPœ?g-úó$r?ÊÖlM?|Cqaµ?H§À©%Ï	?JÁÑÍø`~?…QDªÏ®?{×Y!h2T?ïþ5Q-'?õÅ¿²?pÙÒúöC?"¿ÝÜÏe?"v/›Ì…?p|ÎRm?ïæÓÜ`""?c
‰v?VÏjžrÞý?RGþ¸×sV?[ˆÜl+ê?Z®PÿW©¬?ïÀâCŠ!	?ghèNA?mVà¦7P"?ZæH6¹N?pãmùÞý?_ûíXWÑ?ïï{¢Û>?V+M¤a?5¨ˆí^û?*SѼK¿Ç?[ž¹­x<?TjªCAGN3FGL J1509.9-2951@tù_™Ã‹@8F߸aÜÀ9›Ý÷vÅÀ;|4*©÷¶?îRJ|ÈIþ@ úô¨^@@âf'†¿é
7a|X¿ëኃ›¿áeEy±Ç¹¿ïýl*±À"AGNbcu?ïü¥úÈU?"æ¤ÝaÉ?"rÿ&_õ?$IYá?ƒZØ4}>Ô?aԚò@A?ã¾zɗ/©?ÆÚ#*/1?Ò¼èMܬ¿?Ãå
ú7œ­?·ˆy@¾?¶!Öã}É?ê¾ôî¶Ü?¬Jù‹ˆ?¸yÏ2xs?£ôZ•®Å©?±Ž‰^ý«+?0ò2¯L+?àÐ?Töô¶?»â^âìý?ÒÐ0äR'?½îÜþ.Ö?Ç ãÿˆ%?°7
ˆSÌ?ï}Ü[­r6?‰–ækA]?‡³û:gh?"úÔ0 ?qª²•†`?qR"–W?éÀÄn"³?»/&ɘdæ?Â̄Ú¬3?·ðyËl&N?¨Á¨¯Ë¯ø?¦MFÅM?í¢^« Æù?™ø Qrþ?§¿L7Y?"2°áœ®?¬«ñÀ4)?‰ázêèýÁ?çœVxeJ?«+yzc6?Êö†Úz4?©&²?""œ?­Þ¾]e;?•É&±ÿ|AGN3FGL J1510.9-0542@vÿÅG@EvÖ@†À8VGõbÀ:õÇþ0òç?íÎû?0å@<k~ÿ@gŽß×@™¿àp‹Ð¦¿æm¡v»P׿æ›\2ÂZ¿è‰.NjâAGNfsrq?ì§Yíuþy?µ_­ÓÐ?°AƸ(,?®[]æém<?¥ÕSá?¦vÞٔ±R?ê	\`º;6?Á|¨ý?À±'!1?»s|àŒƒm?¬£ï´³of?±J‹C´m'?鄽ϖ"?­E"ûùUÚ?³d¿ÖXâ{?ŸwžX?À:«œaü?¥é]AÈ£þ?Õù®"tãú?°ñõÅ!YW?Õ¾UÝúi
?·¢¾"d{?ÔGûŒ}Ò>?³
Ü°x6?ï.xI£ô"?¢P÷‰üÓ?ŽŽe앀_?–Ýrvö?…Ó‡­Ý.?€TíZ?í€Ê*3?¶Y'"¶ÙR?«ýõ÷ƒþ©?²®å.·0?—êÓ°Ý&8?¡ª#Çé?íiù:`p?¡ØsF)«?¤‡'dƒòš?'¬z´áz'?«Ïfjc?™ž×""Y?㮓{ÈMa?¦$SfAn?˳%"¯Â?¦>ŒZP_g?ŒŒTÉÜ?¡<:;6Î#AGN3FGL J1511.8-0513@v)ä p¸Ð@Epà<ìÀ9F ²'/À;.¥öŸ..¿˜p'Á]O@ãRi.lÐ@EÊ`‹Ûì¿ê½€i¥h¸¿ÜüD£aÞ¿×â†G'K¿á8;ÝÉÕAGNbcu?ïô×´ÌÙ?U¿<»""?JZ‡*Æ5?I1ÓXÞ?BF¥ý.®?HSt´ªú?ïtywì?'¤]p]0?'û¯ì?ƒ¾uO5Ç?ƒº¦Ïv?Š•ȱn©?îÆ#?A«¾?ŽÑ·Œ+™w?ãý‹ž"?,=Ç/?—2´_±«?†jpµjrŸ?ìCBÉÂðð?¢jhY¢?"áeSÍx?{ÿýEÏcÉ?»b-'ÖD×?¢6ÕÿüO?ïùH{?D´V,?@$"°…½?<^¥ûTî­?5vϘu‰L?3À1éq?ïÒd(\?tIË\&Ÿç?d÷Ñi³Ýœ?bÃý™Ü?h¤zXŽÊ?n"g`£b'?ïmï!5"Ç?_)^²¸°?'†Šô\?wîÆ0U?'s±%šúÞ?n£§aß<?îÉ÷gLŒÃ?ƒ¨zpQ&Y?wà4'äºÆ?bu0Õ.? d'üBt?Þ¯VOAGN3FGL J1512.2+0202@¤r¿#N@Gý}æOUÀ8zFgÃ]¸À;@¾61u?æ{S¨)Õ@ÌZÁ¶%@™ã KO	¿á½-'³N¿ã'÷­ßT¿â[eé#¿ã†Õ½à:AGNfsrq?ïñõOÅ1š?Râ&TÃEÎ??©´¤vê0?;oÂ1	?T*óæi1?OHIå̾•?5òd?¨b¿ˆƒ¬#?˜c_ømwm? E‰£¬Ì?"IY^lÒ#?œ#½5?ïÖº†t?'(Ö
Ñ?…Uï-œ[Æ?|éʉӊK?"º1¡Ë›?Œ6=…šÔÅ?èùrQx?®Ú•¹ðd?³­+EÙi?¢ð9w:·?ÂC¡Ø­Å?ª7<%vçP?ïùžCz??ZßU?5K«=ä'?/Á®ÿ/4i?=ÀÇ(©Ö?6û¯ežø(?ãžJƒ?'"0ÁAgú?Që«T@?Œáú–ÎR?yrZãíÐ?¾:#™‡?ï¡Nö¡÷%?y>æ="¬?s(\rI?lÅ1Ýã?|0r¡x¯@?rõŠ7$O-?íŸ>1œÈ?'',g'†¡?¡\*ÁRMÞ?"©'6Ùú?¤¯ò"Q  ?Ž'è•ðAGN3FGL J1512.2-2255@uH^`=Wy@=xœ \–ÚÀ9â¾÷!À;d-–;@H?«†9¸¯õ¬@
®µëÓ?þôÿÆÊ)?ïËuȕ@Ö¿åïÿµ_ü¿Õ"'
»¿Û&ón¢AGNbcu?ï¿é¾¹Óe?zº²™Mw?YeM¦0?]×ÄÊ
Tâ?y±ÜuP'ú?w†¢I(,?ïKfÆ2©Ë?¡PWªbžï?'u©A~¾?}£wq"/?Š°¤çÅ:v?›%ɦð?î5Ùfõ>?—a³*hÎ?"wŒÈ]¤?ƒ9ÔFÉR?¤f¦œM?'d=¨hO±?ëŒKø+?­ˆÍ"x±?"+8'æ£?9×,Æ?Àœ:TK?­F`¥pã#?ïç¬dÕö?bJl
°ôÕ?LÙà­x/	?G3þy)D:?a#aÏÁ?]Æq?e¢?ï¾À…ŸD\?ƒÕLHè?nì±Áq
—?u'¾"ˆ?q)d\ä¢?|&/:êZ|?ïEjÞâp?'ê(­¿/œ?ƒ'Ý»š
õ?v'qŠC~È?‹ž‡-õö?{C'÷?î¿nùÄñ?Vê‡ÂÝ?uë³öDÈå?d=s⨑¼?¡K™çŠLÑ?ŒlÞ0¿"éAGN3FGL J1512.3+8005@\ýÃ?…Q
@A†ªšêÒÀ:›Ò‰¥/ÐÀ<*y®AÇK¿'&†ç
@Œj€ý@ˆ@ò`…%ï¿ë¥ìp¿äø,"¿ã'l"	ì¿ã3-ÇcZAGNbcu?ïÛ#A?|°NËïÉþ?qƒË/ÍzØ?|†ài—µG?-R‡pXÖ®?&IfRFû\?ïðFN™?‹voK{ú-?vÁi.$P ?xp"S£0?€ØPÒï¾?"€Ž©Ó-?îrÎïą?ž9F¼Š±á?¡ª›aªEã?ÖŠëÊ̔?Œ¢Ç´›9?wòœ‡»Ú?ï¢P
j£H?}‡:|ÞÆ?e{W:Tµ?_dÊÀ½#Ô?'&^†A¦Õ?{ùU¾ã?ïêäxBºm?r˜ç­üº•?dHÎó:I?r‹s±¤e?W+d2?g#_ïô?ïÜ°Z®ÕÉ?k´é‰Ï€?^êÊ'ž?YÑ?Q¿Z\?cÚ?¾gGx?b`få~?ï"iÎižÄ?˜VÎ¥þ?•ùמ—BB?˜µ nñ‹"?vãºCÅ?cAOõÆt#?ïï˜B›Iâ?VÌ5Ú
?Iª¡"‰{?7÷,Óïœà?Sú)ç"	?RúÀ.emAGN3FGL J1512.8-0906@uôŸ`—Ì@D?ßéàÀ5nV·œ¹àÀ:¬²{ï@_"͊aî@"$åg£R@" ¿M¿âR´ü²©Ç¿æPH	"
@¿æ—/˜¿è4š7½ö4AGNFSRQ?폅zdt?¹|îþzïµ?|6êþ‡?…"õLÊí?±ÀríЀö?¸Ÿüi|¼?ïÇÖ¡óì]?}dn6bìJ?j$'A…ø?o¬çF!)Í?nÜûÝ ?rá[†'ËU?èê&qPG?´ÓO¼KW?³K‡wý?¢T3‹'0›?ÅöÖÝ-(h?±ãD&ñ<‹?ïø梥 ¨?`ü"‰ýH>ôb·hÊ?!|Ã0c«?KÂa¶#Zº?`åô‹þ?ì–e£"U?Åß6ø ÌO?v¤ƒ¯ë?"@l¤¿w°?¹âŠ±Ù~?ÅgeÄâê?ïêŸZ}?b¿!8jòÁ?T#×W˜?SBþ1ë?VQŽhe%"?Väh])+h?èm¿MÞ/K?³ë?ïÃ-?²åmŠ³R?¤Ä¸ÍaS?Äւ'/Ü«?°t@'Ù\?ïþœJ£è'?C¥ð+ý>á«ywòôü?+v»F?%  crÏ?C†ÖL	\…AGN3FGL J1513.1-1014@uåóà7Ý@CžŠÿ¢âîÀ91#ã4À:¨Â<Pg¿Ý¤}6Ñ<7@.ëBƒ³(@ƒ@;ÚL¿çÄëçf£o¿ê‡a(¿åõ—1´6¿ïý°<÷'AGNfsrq?æK¹i˜Ÿô?ÊÏwŠX¼?¡Œ¼'?Ü.I1?Ñ7;w¥S?ÊÈj…{²?î~€Öv'#?­Ë¡tFˆV?™F²¢ò6R?¦Jó(¸"I?–é2ósB? ;ÎöéC
?à˜ó<ðn?´—"½A•?ÂzžnaÿÇ?§DóË°«?ՑtâUA?³èP¬ñT?ßâÚì±TÝ?Ã*ÅÑZûú?©hjS0ú?ŸÀŸÐ'é§?ÜðÃHÈ#?Ãn>±‰?æ.X'Š©?ËøÙ ©T?±XŠ‡Eš?´GÇO@wB?ΚX³lËÓ?ÉÙÕSjG?ïuö¸ó?í?žóúEþR[?'yůET?˜x»[=ñÜ?€×úit?‹ŽW¦m0?㓌fw¥ ?´0Ç ?ÁYßɘ~«?§ÛjÏu¬Q?Ð+÷NDuj?²ø ¯\?æ$>úè?¶ˆ7Üx,?šmí'ƒä?‹ù­éMZ(?Ò0Øõúîs?¶({x‹ëAGN3FGL J1513.4-2549@u-ÿ¼ä!@:÷_f—åÀ9®P(6ïÀ;¦¨ñü1>?ùX,)(ÃC@GõM?ôò¬O©¶r?ÎÕÐxö-¿ÞB1õÁÛ¿éÝk±åüÛ¿éVcCÇ*!PSRpsr?Òò#'ˆ0Ä?ÈTp\Uã¯?■Ýèul?Íñ[ºo­?¿†jʛ'Ž?Áuö~ng^?ß!çDñ¢?А‰–}k¢?Ù ¼"°"?Íˬ"qa?¿-àÎawi?ÂƽÃ^Rà?ԕ­#°r?¸µtê®L?à!²ß)µu?¸¢ÓŸçÌ?ÆMÚ;ÓÉI?°¿<ƒæj]?Ñ ž2R&?¼*°ä?㶬Nýê?ÂØl¬ëIÔ?À?èê ?·é"õdôá?ÜP|3$?Ï 2‹©¨?Ý9¾të?Ðt›š'?ºžKÌÈ?ÂzáA<Ð?æõ¥›ÛhF?Ð['e"?ËÚµ-Hãt?Ës¢†t›*?°hÃ#Zí?µéøæ2ï?ÝC¨û{$Ó?·îFöݸ?ØÁYêy?µ[_e—é©?ÃõûÞ÷ág?¬Xû%È?à£~âU—"?¶}ž6By?ÛOo¢WáÇ?´Ÿ‹°ìª4?«L"Ê{.?¡Qþ½o>MIXED3FGL J1513.5-3233@têµ_þmY@5këß·‹À8úaPÀ;[ƒäün{?ò¬»y"@ÃæÄŗN@¹áÀ¤ËQ¿ßn [·ƒ1¿æ:À&4Œ¿æ×G<Tš¿èœÉ@j:AGNfsrq?ïõq‰Z1O?NAËG"Á?Ks˯ø ?G5U'ý?=ŒEþôò?8cvÄmÝÈ?ﯷ…4T=?ƒÈùÐç?p?©ïÃ>?p%¸ÏQzß?xý¦˜Šm?œ6+´†?îà:á¾e?[¶å"ç³?'õz‰‰?"öbó?RP?'CË>©Ê?"û-S{ë?ï™Çî&õÉ?" #¹,?a$åÓŒ?d"ß#¹?…Dÿϳ¥í?'Û{pI£<?ïûµÀ……?:áÓÇS?<b¢¾ÃE³?4õØ¥RÛç?&Ï_¥2N9?"6œO{Ú?ïá'{gKá?fëéd)=?Z*ǧ?S΋uª?aqÿ7Š[:?ab£Ýñ‹?ï^Û
"w¨?"±f¯f?"¤£ÉE^?vòL­?ƒ¤™¨ä´?xä­Š˜?ïåõ(qÊY?cBÖµ?RÜßz]˜ÿ?LßEÜh$?`œgÇgò¨?`˜?I'€VAGN3FGL J1514.1+2940@GÒtw@MQ™?׆dÀ:/àÇU"‡À;­ä9ÐÜ&¿Ý"žfC<&@w€*@Þ§ªÿ¿éªASv8…¿ìLû^ÿغ±Úá–¿æ3ɖ¿þAGNfsrq?ïý†À›]‹?7,ð74? †ù7aÙ?	é¶Nߧ?/ƒ°ë½B?6	)­w×?ï°ZM7?ƒrN3-–?q"+AUïy?sÙN³ÎB?v°†*´"?{-	XÝQ€?îüÜëH?@Dé"×?àÞ(¡(?v‹Î^A‡?˜l~ŠGâ°?‰¢"ÒÖP?ïo‡Ù	ê?†)XoÖó.?Sìfïšüt?Sd'$7¾ò?Ð>s¤ð?…1ƒLÿv¾?ïþ‰"܁~?(.6Bd…?&)ÓTÌO?ßået¯?!¤GFÃ=?%ëw[œ 9?ïâúÒ7	?ht†ów:?Yð"4R}ˆ?V½À±à´?`
6fDà¶?a¯w6'?úlJß?…'%L»'?vܻ̓þ®?}›.ªòa?"tÿyNøÅ?}"Ì@R†?ïå-8P?^waÌPãŒ?@ðiêÉ!¥?0÷>¶È¦?f¸¸G¡€¡?\vFüéH!AGN3FGL J1514.2-4947@tS°€0<@6™_·ö|À7ßÇËÜÀ:à)q'@å[½•ø@±aˆŸ?üûòª,¿ÓÛ'~Z¿×Š
oª1í¿á"Á0¿îö¿ëhdj/@,PSRPSR?uä?N¼?y¡ýü¨?ï:Ák^?—1¬÷úŠç?"Cx^´?"ß'Ÿ"½?pÅîÎ2µ*?¨_Ë‹I¡?ìÀ;ת?ºŽ\hz•?ºåŸ8ŒZä?¸'ŠÃµ?ªb ×:4?Ÿ…³ôéÀ?êö3o\óæ?¬œÜŽ)3?»a¶d'¶?¤ÃÚC"™j?~ü°ü?xW=
mÞR?íTžªûkÇ?¢ð‰?³k?§hlÙ? ¬¦ÆæŸU?jv#lD€?o%ãiq]»?ïCbY«0à?š"|ח7?"DðbÁX?˜ïtž`É?iˆ«>kx?y΅f‹?.?ìþąoZ?³¡‡eï°î?»'E"3Ô?³oG˃'?ºp"aùð?§¬DÿÔÛ?é`Ñú¼§Ä?°ü4O…&Û?ºˆëÈ ÑÃ?¤Þ¥Q]?‹7âÙ?yï\@^?í´š8ÐÖó?"·e,`£\?­ñNx"L"?'BÌ`ôÀPSR3FGL J1514.5-4750@tdñà'Œ7@ Þ#ê¬À8ÅÅ.î*À;-R,¾?ãË4ôJât@àjR¯$p@£q ?[¿åݕH•ßÀ¿ä­8Íw¿àõ6â%Šº¿ëF'9LAGNfsrq?ï£Ä~°ÆB?€Ý;ìû*?€	ÊXý"?|uøS[S?lX¬[i?gf¸b?ìP!è ÿï?º"îôŒ?›å¨°'¬?›í
ßöØá?¶…†½‹ö ?¶-û§ì¤?ìôqxyu?¢
*ۈÂÖ?«©5üÆ?œß;5÷c?¥ÂìƉ´?'èqàÁA?ëlL+Җ»?¤åÀ½ä–\?Ÿ _¥dÐ{?ë‹YŒz?¼µ†¹[ð…?¢HIWJ?ïáߒ(?j"šïâ~?gô<ۄí?gO]þfa"?H°Ävû[t?E±{¸÷?îó Õ-?¤?R/µ•È?‡+øΪ¿Ô?"ÔKóÓ´¹?›ó•oúu? uÞ궶™?îìûÔ!Tä?e´Ò¿†ç?"dA÷t«?ˆ¡?fºx?‹øÐbÑ«?}¡°{³x?îjNW?ŠWêaX?'îG{_ý?wš€û
H? g*õ`ºŒ?†·#ÁpæAGN3FGL J1514.8+4446@R‹UŸÚ%{@L7W`9%»À9J\OÝÀ;ÊÅ-œ}?íúgPàÜé@ÐîÕÒ°@¶G_eY¿àa·ã[¯~¿å"ÐèBþ¿å™‡¿Á¿ëU'Ö¢}]AGNfsrq?ïµúÎ<ä?›Ë?rËhc?œ[61•N?šfwS)ºè?m—+¾hÕ?hÓÁ¤ÍÄ·?ë~ú9 ?¹—͘
©?»Rò[±×?µìË꫃G?§¢,.>ÿ0?¥pZ°ûŠû?ío'ƒë™?£µûç óÜ?¬«‡gCÚ@? €UŠQüB?˜Ä‹<p?ˆY6ÝI¸)?ç_i¥"«?±ŠbÈÎų?Ê¬X/ŽZ?«G3Êñ?®×XTÖâ?¥]Ó+Ð?ï°"šè+Ö?|[œŽäå?A™¹‹7½?y¤¢n¤ØM?U­ûܝåÛ?RãU؀0{?îZÿ¢Ñ?¢"úI^x?¢Za¾iE? cè"N´?Ö"ÓŠvÔ?‰#S5>ø¥?ïÀYæ•?,þFߐÞ?"iû!‹Ü?ˆ!Ñ#-2'?'»óKg¸›?pôx	ùÁ?íu²Í¼?•ÒúVï¾?±/.1ÒÇ?Õèz3j?‰BaÏRãþ?"²Ÿ7;ÕAGN3FGL J1514.8-3623@tÊ # –@2Ù_'F—À9ë>nИ3À;‹<R–¥É?ê©idð@oèך[6@=¸¸ÇÝ?âºT£‹¿ç,.õ¿gè¿ælõùÕ¿í/_[&¹ AGNbcu?ç˜sôf?Åbõÿ²8ˆ?ÎfÙï±9…?Å7{õÍ?™ºÏà'«#?˜‡S;©]ä?æ¹dDo"?ÈÉÍ­ð?ÅÁa>UÉ?½se¨ÐÞ?¾²¿¼]?Àh´r@—Ó?ç -î…?´ðèb£?ÈýÀT€?±ßÇ÷ºÁ?µr`? :TùLI¿?ßE…n¤?¶nþCõõ¦?Õ,]²sìG?¶ŽrÊÒëƒ?Ç:d;$*?²É;y§¢?êŽþ¨'û?ÁQÜÀ¿?Ä3&pà›i?ÁîJS"Ù?‰
îèñê•?'í?ë秭ß?»	ú³B•¯?³–‹š*ø¢?¬ýÕ6~"?ªXvÏOÃ?°ôŽÐF?êç \´ê?«
<`záj?¾É…ÍK€?§gÈ£2Ϫ?£ûÜN—_?'4'÷=O?è^ö™`?§Ô–±¹Ÿ?ÅëP.i?£™NêûŠE?±2"r·Y? L¸Ý…yAGN3FGL J1516.7+3648@M×­€k`@Lô¯ÀL‹ÊÀ:s[Ÿc6À<
ÅÓ´G›?ã'ã鸯£@Ö;‹qc@שjÄD¿Ø‰Ö«Ñ]3¿â­vû¿åuÒùüI¬¿ïþ;g4A¦AGNbll?ï'E<þ–§?'Nw¤»?‹òÒ<o¿M?±PmÌN\?[ÞóŠå˜i?`zGÐÁQƒ?îC·«¹'ï?£Ôˆ¾6#V?¡8øHh´?Ãý†¹~?•˜<Ъ?"©Xd¬8>?ìWÀÔ?¥!ÕÔà?±Á´>–?ùeE«E?§Dt㧑?œIî÷Êy?ìRKYo²ë?¨¦ô£îs?¶Cl­¦Œ‰?¥xٖÎ}?œ¨â·¢s?"pe€¨Ö?ï"qCº
?¯ùx¦½?‡æ¸äÁã?«P"ܵ;û?Wç±ä@í=?"×çGÎQ?ïéŒBk?…ºd?o¬‹?'üëÌ%?¿Aü©#?zbfô)?u£T0–dH?í'ØÊd›>?¡ú"mœí_?­sŽWœ.?›O'7Æ? å-ö?—1ü'n›?ï {‰tn£?"Sgô–?–ÕĺV>?}lW¶²•?tmÌ% å˜?t´D‡¥ÆAGN3FGL J1516.9+1926@;՘Ÿž–Y@KëÀ·pDÀ9Öï
wÀ;µ"'±ÈÀ¶:¯³â@ül¦œau@#ìÀ24±¿ænž¯¿1¿êæíZ¿çû÷–5GF¿ÜÛý`':œAGNbll?ïñ¿T-ª?V§S?9ö?Dñî'Ãζ?FÉwÉôêƒ?R`‡6c?P2{ä?øv?﵎hFÕ?‡¶¬¤ä%"?qåv'<¸?ƒJa$¤ü?sSókH؟?u3*èt'¶?îÛå™w`?NA_#"?Œû•ä¸ŽÃ?zjp½©ƒ?Ÿf¸cҗ?‰&"/Ae?ïªè®Õ•ô?€j[ߌ?'¿BŽ{Á­?0fälL?"æ×I"V²?€AV?•Ø?ïú"ü:'g?@íbxoh?/ϱ_?,¨ð"'ZÖ?;x"4˜O2?7®_¥nØð?ïæ^¿[¨¦?m4]É?X	;2É…?`†B wI?[9Eïjý?aʅFÐÓ?ïk3ô4€÷?x¢îˆÝe?~¥rT?iür¦–zQ?†*01{®?rÈù2ÐD£?ïó÷oHôL?PìfX7F>í[¶"t=õ>ír=¿?O?WÖje½‰º?Pá|ˆAýƒAGN3FGL J1517.6+6524@YÛa»û@F³'Àa"À9OŽuy)À;L	ÃÎ!¿õ`‡·™ß»@sIcKSæ?üƒ—
&Y?{­5F¢•…¿ã-dÃ2¿Óƒª3ða¿Â~	ZÇ¡ÀAGNbll?ïù*–à	s?AÙåþR>t?.ÐÊ2Ò@‹?%À¬ÛàÅ?C¡rzl¬?>ú¼½öy?ï·|Œ <ê?0ÙÊÒ
?mW"ƒU]?oAM©‰WS?u•÷ÆôV?zRfàwå?ïDòmàr?ƒ*塤éÑ?ƒôîbw~?ymšmð›?ŠÎmÍ5ð?z2ÂJÁÝï?ï²[—€d¿?xúWmNà×?_ìåÅÇ0?
Á«óP†?ƒIº2'5º?xï/ö¯H©?ïû•
Ý}
?4Õv•²?.ãdç©Ó"?%_ܧ}ã?3åßýç¸Ç?,	§rå?ïèÍÇ&M?bö9Uª¸?V#,ÚCwã?RL ¶J&¯?YÅ7y3]©?YÏe°@?ïžÝóˆâ?vêä½ì΍?wò8`~xá?q¬¡AWZÿ?xžÍÜ$'8?j̄͌"¾?ïñ²³­'Q?P""Ô"Bm>îf<·½È>ç	ö꨸ð?\]ÌÒ좆?PŒb4	ÀFAGN3FGL J1517.6-2422@uJÑ"Dž@;"§@KIªÀ7es!_ÌÀ:ÔÖ-žž¼?Õû¶_"$m@eÓ|"P/@å±_³ï±¿ã#oڔœÁ¿á¨ãîžÑ¿à
¯€ƒ"¿æ"YO@tAGNbll?ï"S£d|?†¹¨Dç—}?ss0z¤gz?nÔŒoå?…1¤Æ)H?'ˆ}|oÞ?ëºÕ©jG?ĖÔI?ºí "	¸?¿š"¢ä"_?ª
OfÔý?³š³!ºkÊ?ëe¹ÏD?«ŽGp ß±?¢Nè1·p
?–1É'ý?»¯úøó\?¦ÝbLI†f?à®u¢»Ï?½ã?">,z?¼Lð¡ür?±dèÓb?אÈ('	F?¼ÆWÓ%¬b?ïÞ)¬²â?iÔ5)3&\?TMš
ñþà?R^ªåÜ:@?gÙ	fq&E?e8E¡^ÜÈ?í'ÆUÜ¢Ð?¹((è"o?ªÆÛ7O¡?´B0Ä´s'?˜:ý‡ÎÅ?¤i)‡ŠcÌ?ìUå¶cåê?¨'å‹®¡?¢¿gZ=tf?™9}oÚgò?³ñ 0	ÿ?£Å©ÀHÔ?膮9'­³?°ŽpE¸F?ª;ûvE?˜}¸ê!.i?ÇVH<•î¥?­"y|ç³ãAGN3FGL J1518.0-2732@u*­ ‹]@8ùx¿.~™À8šRÙÀ;$C£Ã¿¿À€+q'Æ@"ÂLÁ#Ì@‹Ÿ°ßÜ¿ÞcS÷ÎÙ¿äâ=X¿Î{¿àÃQ,(¹¿â>*þ0rAGNbcu?ïüD	ª×?4ij3Š'?nlpFß?
.º?•*¦?8Ã…ºÆ?2J÷ö}?ï"ä³jÈm?'Ä]¥h(	?uƒJÝ‰d?'Úy†Æ…?€E-×Ê?‹QžÕ=Õ?ïXøÉÍ5u?ƒ\Ҕ'	ç?{ÏÚ}úT?kícIi>'?Œ:e£ë#œ?o"ìõvæ?îs@‰)P?'žŽuú:?`'ó(Åà¹?XÖsËóî®?§ÃÈ8µËv?'d×ù"Cz?ïþŽÇJj?Þ2ûAN?
¿Éà)ÿê?Æd+õÙ?G<ûU&?°¡FÃà?ï×"¤xMw?sqHì}i?`P©	Çø?W…§¤e¦?hŒ²Àv?pD‡œÖŠÈ?ï±Êà¹hÂ?p<_d9?mù£¦Øf?R{rÇÃ?x½ÝžÊ?m#ÕîA».?ï˜èÁõÙ6?u
_qÒ¼?Mèκü?;x–L>Jç?‡ô°éæÔ?u"Ã#`ÃAGN3FGL J1520.3+4209@QG¿@OÂ@L_×ÖìÀ9³—>u‡À;ÝWªå?ì/xB~L.@5¬µ*D@ýXÌ¿àv›"_aÔ¿è¿\"ÞýZ¿çCvý<½¿ìPa¼Þm3AGNfsrq?ïòFNª?Xsv AÌ?TÊYH§Sã?UÓ¸íÓrÐ?<$ijtŒs?6Ö?ÚÉ?ïG P ?˜>–"4"K?«¢ýèÅô?'Ÿµ[yË?‹ñú|à?dëºA?îZs¯WÏ}?—Ùí'Ó\?ŸBëž/f±?'͹Ô?•nžn?£¯?Š¹©"sAÁ?íZ8=3<B?¤]Ú
Sê.?ªG×±·…ƒ?—º…Õõóë? ¤{ðT?œþ4ŠÍ?ïôñù¤h¢?QN϶ëì?Qš÷ØCh?MÔÄYD©2?2TûC-]?0µ®»Á²b?ï¨ùÏAúª?{ZÉm{gW?vç:«‡`½?nQrµ
?t›Ý¥îi?t¦KΞÑ?îͳ+ˆfc?"Žçò"á?–øjq~l?Œ˜½eY¾?Ž¡úE"Îx?‰HÍå€Â?ïK"n?ƒw–?j?'_ü_¤É?u……®\̘?t¶
¨(7?z´½ÛoAGN3FGL J1520.8-0348@vaä?åÉ@E@Ì?ß À8ñzbœ­JÀ;B…¶Æ?ìù×	Å.P@þC"¨"Ý?ýXà¨Ì½?æ6Ãì±ø¿Ø¼c,9ͿΕE=-­¿à$¡Vk5rAGNbll?ﻨn!?{(jCsÿÍ?véÒ
ø¿Û?t³°³Éëü?f"E¥ø¶Ù?oÙ7¼ÌMó?înª:%À¯?°uÞÒ©rº?¨Jé0¦S?©µ~§zع?"'mÓÏÏ? ÛFöÕ!?흱Á®‹™?žE{÷¬Ó?¡*,!¼«Q?"½™¥™?¤ú·¿êÿ!?"ÐÃk>[?æ¶ñôy
?µ÷+W2$?±ïx"Ê‹?©ðFõ?Ì,|!†?´¢o¸?ïÄe~Ϋä?z`Bêo?ttñw.¾7?qm@ýKœÃ?b°ÿžH
?n]y?'‹?ïKÚåÐe? )^ÐÉET?‹Ïðos";?š>ÿy…B™?9V
•.¢?‰
…j0Í?î½F³~Ù5?'Y˜ÞÄØ?"•!k³Íå?†jžCkc?"Â+PCm?‰˜Ò (&€?ë—Þ%A/?£F‹§(þ?°ÈUˆŒp?•Ê'»a¿?³<Fiƒ? e•Ž'AGN3FGL J1521.1+5543@V‰?ßéà@Id›`C6¶À:{7ýJCÀ<#ǃ·°?á&D"He¹@
È—ý¸'@]+éTm¿ìQßÅC'¿Ö.î"Fe¿å=äð¥¿Ô?Áœ"[AGNbll?ï×Øocn?uM$vY?kêkQÛ?ršúò÷o?ZJ2KPé?Sü{¡AÚ?ïjá[‹R??–Hé†te?'–À¹2?ÅjQÏc?'±¢Sÿ?‰;¸"åY?î‡û3èdÙ?'":dpf?"c^"]?"l¡L"p?›:ïÝKŠ?‰v•ÆkØÃ?î² ^.ßg?œ'á®KÑf?–sÅ7ä?—oÐ;yû/?"8Õn÷*?ŒÙÞÃð/?ïô_-À‹)?RNI	ld?Eá'Ö9â?FàÊhYw-?H¢!`öA?Bʚ;_U?ïÕ!"B'Ë?yBª¼XÂ?d$²1''?iðøcq?fº+¤ç]?oî"ë;?ï`"Ô6?~2Ö*¿RX?'5hª~è??r¾–›
ë,?…¥bXBiå?ußð[–Uw?ﻞ÷§kê?vÂÒ˅ú&?w¸v–AÅÒ?pKµ•Ÿf?dðþµ²g?ekz{‰÷°AGN3FGL J1521.8+4340@QæïÝëÙ@KÉN ƒyÀ:$ìH"ÉÀ;×#{/K?×ÜŒ{›@u^>#Ò@Ú÷àvͽ¿æß+‹7ðÌ¿ëš{Òðd¿ç^õ }ùֿڕTV0ŸAGNfsrq?ïþ!ŽE'§?%-hD{ÛV?Tõ¬Ùš…?4$Z¬†?$¼¥ëã?!ÏqÂß?ﱯã2ù?âªÈSµñ?qJ¢ƒ×Ÿ?twÖK1ÉÕ?ušÃ©¥7Ø?xUê«Å??ïHè€ÿ¼0?€ýZ6u?}æ·­tx"?rHŽ ªx?ŽÒƒÚeÛ?y&›Jøºz?ïOÎÊRõ?…ïG‡fŸ?fžŸ+l?g¿¢Š`™?Š¤…óÙÝÖ?"ƒïB«fÅ?ïÿ<íñ'?E°²žïç?×û||a˜?ç8\qòç?$Çq£$g?Ú5hê?ïä®lÿ?céjLÌ?X×:ƒ›jÔ?RµWÆ&Ÿ?]̏[$?\n¼—éŸÐ?ï©ìyª)Î?rHÝþD1g?pmŒ2ÆV\?hŒ~í¨g?zœ7
ºQ?i+òñ}?ïè
ESFN?d{-çTp?Oÿ¶¹;l?J<üpT'?_ë™ñJ1?`'ªç9ª…AGN3FGL J1521.9-5736@t VàL'¿Ûd _þº¨À7d˜$ qÀ:D˜n#Ê@d—.Z[@Xç×Nl@=Ã/@¿Ï•¦'Gã¿áǼ¸é§4¿è}M÷7b ¿í ÞW
ØÜPSRPSR?AÅÌö@ªò?; óÏ
O5?ì1¸‡£?¾Øjî>@?¾SÖ§þŒ?¾Ì8I¿Þõ?,Ñ+݀º?E½–egüÔ?æðqĵÉr?¹Ø¸ñ×&?Ò'S1í?¹"ÛìœÃ<?ƒO{o5c?v2˜›OKÍ?éÈxÄ?¶´«@P¡/?ÊÊé‹ýØ?¶RKӅQ"?{'t0­ã?n—́ϫ«?é÷.N‹Ã?¦"¼lÛµ?ÇJªEkø?¥ø~F ¦?8ÆÕbÍy?:
DDž?êÚ|–\+?Ä_°¨¢d?ÇÄ2£°¼?Ä[F.¯ã)?DG`Tê5?\0OAžh[?ç—øÏßüª?²E.lÖÁ?ÐÅê°bˆá?²!‹4vá%?ƒ¾Þºòm
?'ªÈh¬?ê
–a^rZ?±:뱐ò†?ƍ¸Óó?°ê𘩻˜?…فÉÀ¿(?tÑ×É¿?êwTË3p? ‰½+?ÆtŠ,? 3cä鿛PSR3FGL J1522.1+3144@IÓßæ…@L'ßý`éÀ6FchÀ:£ÓöeM?û¨w³?Ýæ@…éµí¸@~ÓnQ—L¿âN¬Œv¬–¿åʍ¿	¯p¿æ]J "'¿èÏÅÇíAGNfsrq?ïîþûä=?ZtÄêŒ?W£Ñ£ë?Wºgћ?D¿é(‡Ã?BìrK?ïÅV¨G ??€,ÂÃkõ{?kzèúåð?t%Í!ÝQ?o'ÜÆEóJ?s.³¨S½¸?îÐb‰jª÷?˜]ëšL°?'ˆ':ÞK›?¤[ª€?"k‡í†?›݇ì?ïɪ·ŠV—?ƒDŸP³?I^@¢\®ö?`IçT¸i?wþÜ'­<?'Î~›ðð›?ïò™óÊ?V#G_¿s?Vzå­þ_?TvlsfÄ ?5·¡hhÛY?4.ú
^%7?ïä¼?‹Ü?r¼çzÁ¥?Wá9[å[?Xú]yŽÔr?_†ŸÚæìå?lÆAµ…r?îÿp29…?"X×£
¸Z?#ã>f2³?‹R£X‹?Ü-ª½?‹»
ä|Å7?ïö_6ªá?bÊrÔ¯¬m?0'
eÁÁr?:ÅO¿šÄ?No¢ÖdýÍ?b'ÚLAGN3FGL J1522.6-2730@u9\_|gZ@8f6îÍ©À8$l"}ÐæÀ;žîm0…?ò³üY,l@Öâ'ܼ@"à)ËÖ¿Ùkë[-M@¿ã^¢;˜vH¿àTË«±ì¿æ´œ.ÊBÚAGNbll?ï÷´°\?Fx¥(|h?'µD¿º´?#»´¸jE?KBP4%:?EÆ©Àûû?ïƒé¢¬£ô?ï#xzò?z*ˆ¡!º?u—²ú>Ñ?ðSRv6?ŒÆéì"Ô"?îÆúáe¾©?",€Ñ?Ž¢43=Ž?"Íï‡må9?—ω¶9ÇÔ?×¢fú?î]½í®;?¡®±E‹=?'bÖªX?|a°#U?©nvø|J?¡ 2káEB?ïü¼Œé?+B'Ã%=?"ø}Tq‡?5c–Ä?0ŸžVS9?&yP8Ü?ïßd^ÏC?z"ێu?jD³ïÌM@?a_1Â­>?q
ó҂ëÄ?uø '¸?ïY_;h¥ ?"(ø€/"?ƒ˜jO–?x»|¥e}O?†Æèqa?{<cːép?ïcw87‡?€\6ĝ%?{'§a¬6
?i±6/È2Ê?‰XÞSâõ?~"¸q+'AGN3FGL J1525.2-5905@t8–ž=¿þm)Tc¯À8äç
À²ãÀ:QÎ2þZ?Õ®ËÄu@
½U5'@JÛ`cm
¿æHP¯×ï¿æ©³ÍÍRÚ¿ç
'¿ç-BÀÜ1AGNbcu?Êc@ÒÙ?Ã*¨¬a?À¿ÉüZP{?ÀN#*L?å7-°´µ¡?Ê`V¤Hì?ÑØý^ÝRx?ҕI|?¹¹†Z2â'?·'τ""?ãÜP…Júr?ÑÉëÝom‡?ÏSä»x^?³¬µoiî|?ÇÚ+»o­?±›Uè\#?â4F¼|ó?¸î?CyáÊ?ÚñÄ$Ôíû?Äk†Áz´&?š€+Øw°#?(Ì,1ïä?᳎šÑÂ?Äjn+ñ?ÒԚÊNËÉ?ʝÐéo£Z?È)%qöà?Ƙ98A B?à‹k'|d?ÏdÈqù?݂^†•}M?Õ«à5+Ó:?´ÛžÿÐ~_?±¼F;gxú?ÝF¹¹Zæ<?ӌNŸl¹´?օ\ә‰?¶ÈÊ!Pü?ÇI·#mBy?°rê—Ó~?ÝÕÈOuÅ:?·ÕŽÆº‹˜?â	éQ¬Š?À¸›ðêl?žÇd"Ä?†LùðÖÉ#?ÚúAۀ?¿'Î?ØKöMIXED3FGL J1531.0+5737@VæPß´0@HS?Ýe¡À:y¿ß~€À<¥šXÜ:?âÛ$»#ù@q|ï>çœ@%±ÀVò«¿çíÐ
¿áœF7¥f_¿åRkuwƒù¿µÀ½mÍAGNbll?ïîîZf'ý?b=ßy=?Z‹wuŠú"?a^kó|?>_N®é[±?9vFá¡/?ï§OÃ?bõ?ƒ¼lg:V?sA£'"?sžÔ¿Óö¨?yzáÅY?zóxA{'?îýî4rð°?%'GeÇ?T¶2#
>?…Õ)£Î?—Þ\ã?|äY v'Þ?¢ËØ?‰8)‹¿'?pÖVÁ1Rþ?{/™ŽSI?…ï«â¤?"ä˜ïø—?ïú¸ùdï?EÏÏv€-Í?<»4ÛUŸ]?B©])µ?*ú±
U?(`ÿþÙ?ïà &jg?m_hº(?]0´á=I?]ºÇ?a_¦ârF?dïvLß?ïñý€@O?|µH°u¹£?|Êe'Ófê?vmxñíž?|<›Ä›•½?pµŽŸš?ïì»®ÜÐ?dásxIÊ?Q<0媄?T»n´aq?ULqà§|?]{@ñ•a¯AGN3FGL J1531.8+4704@SýÀ?`@Jr¢ŸÒ˜¿À: NRsj[À<ò¢Ik"?¡øsìý=@
ð*IÏ,@†Aßsm‹¿ëÜõB¦‡ƒ¿Üò4@à¿æI§­Û¿Ø
«(t‹AGNbll?ïªõõ:)G?xªµ)Û?
håJà¸?Œ&)Û&Éò?`àfüq&Ê?bDSû?ï—HŸ@?Ž¦k4";?y>GþbAL?…nïØݪª?{®€Š§?º8~ã?íöj°?™'—',q? Lf>†*?'àÒÑI? J˜ºØuÑ?‹|3¢ÜÈÊ?ï^ØՑ
ü?‰`ՆCvX?{TOÎUv?z*¾E¦¢t?ŠŸ£&"Æ$?"ÆÖM0Ð?ïî^«9²²?bŽ¼µ—?ç?V˜òb…¸?_Ò%v"n?ISn2¢Á?Jbp6˜ž??ïáWv'8?gô{dgÅ?[›ÇÍ°¶º?X¥îCé/?`Ú¥˜úd?`íaŸºw?ï>6'ÊXº?6
H¼?‰©Ô&ä?{Yh˜
Ë?†È†²…O•?n	7S)Ðå?ïãM B?dë?_ø?[^'tê?Sf"'~\?^Bð+ªà?]/~<*܂AGN3FGL J1532.0+3018@Gì:?–îÄ@KhZ&–mÀ:!=ÍÀè"À;´:ƕ?Õe™W)‡Ž@[¦nê?ü>AFœG?ï÷aÐu‡¿Üh‡Š…¿ÑY¤£°@G¿× ‹ŸÊ¤îAGNbll?ïù ­ŸŠõ?EŠƒÑW2X?2å1$ì›?3-\2ìÄ?BtV‹?˜x?>j²çéå!?ï–)[)W£?Š«:H(Í?v—0ݒG¹?x̃mª¨?~T!®¾&f?…!÷ëlF¼?ï1v•?†ú›ÇY5õ?ˆú±f³Ëñ?€kÚ±I?ŠÄ-è€
?v—ÊÚ'Ø?î

?ê·Ö?¡{o®ý?ƒЌ±g?'SÖÙ#?ªm÷Û<}ê? E×t¢g"?ïüPÏêþ*?6ßÔ
È.?#ç|¸"s?%µÙ ì@?3…ÀõÒm?.+8(ëÁ?ïÝiÑCÄ?moçéè¢O?]²=éëL²?U½íd¤?d%wë ?h€¸î'u?ïÏÄìÀ?u¢ûŒ
·T?{iI1,¶Ø?qŽkßÀN?|¯4ó<!=?dЭCÒã?ï"6Òé¶+?zZÐiè¥?qÌëñú/'?cXÁûÌi?'KÕE^/h?v™iŸ:AGN3FGL J1532.7-1319@vHÿ¸²d@@Ü
`:Ó;À7Ý[+J1À:êè'œ&<?èݯr–Aî@@‹Emó@À…Ü.?¿×!R¦ý¦¿á"­Þ8ô­¿ãÄUã4¿ßó¶ËهÆAGNbcu?ïüƒŠÓFþ?0ù?¾Y
â?!²†¤½b?yt(°†?3
dDKð?+Ú*Á]oÍ?ï'IN†)?‡$.<ç,™?mYê3
i7?'cå¼²?pæ6÷'/?tòm£ ?îã­ÈêXé?"ܵ~û©F?†Á*ÆìÒÀ?…É›³Ýå?˜)±v§s™?Žkc|Ê?ïüå¡ãr´?CۍÞЯ>¯Ü)‰z_>ÛjÃ{‡ð?8­NA¿?CÖÏþö{?ïýíؤá? JÐ\¾†? ¼ö?uм—ø?%l‡T£4?Ü¥c=?ïå8¡Ôs?kL¬ò`?U
ÖȤ-?SW))h‡ê?`[\. ?f»Êò.<ž?ï c¸6<Ó?'}('òðÉ?…ž—1˯?†"¨.œp?'${4~·Á?ŒßeaËÐ?ïÿ~ýÙV•?"⧓Ñd>³®pí†å~>Ç¡–»Ö_i?£
Úþ=?"֖ëçAGN3FGL J1533.2+1852@=)@ªÀ3@Jÿ—$tÀ:0;eÀ;¹ãÕ'b¿ãùB¦Ì;@
ŏb^?þOà2ZE¿é†lêJ¿åÞŸ¦Eq?½‰Jl	éc¿Ûù˜áýzXAGNbll?ïòx0Ïfì?Y¨1ŽJ·…?"òLS>—ý?b³¤,=?X±UþUù?XÛæóÏýý?ï²é‰ú?ˆ¡F‡»Û?qÃîævØ?ƒx$#¯õ?tǏ<Ã?xlôÞÛ`m?ïÑl™±B?'RJNO'¾?É9¢"'0?pj6µ2Ï#?"5¡Vå0?}ØMæA?ï€0âÿqÃ?†Ÿ_ 8•?3¤[r'?9ÄxO–]l?V¤sߘ#?††\³±´?ïúÙÇÔaä?;­Ãª1¿Ý?þ"® ?'uÃh‡?@ÙX¥©ž?9Ž'X~Pq?ï倲íӃ?dð2¤åI"?W¶"/TJ?TJø—Åõ¾?]H–Pr¶ç?[¥ÈúvÓm?ï%R«?s>îà˜e£?uÎ=î«¢c?gŽ–'w6î?ÏŒƒP=ð?iˆXêœ%?ïè]¦)Ü?XÞǁÏoŠ?/ûŸþ'_‹?$êe.'¡9?e¢¨Gò†ê?Wµ®µcAGN3FGL J1533.5+3416@K_{Ÿ³@KU@ÿ¤nÀ:lÃÕ­FÀ;ÕòJ4×x¿Òɐjc@¸©Ý3¢D?ý«:ÞÎ,¿ãSÛýÊÏ$¿ç$8vi¿°T÷†½R¿ànG˓RAGNbll?ïñ~N~W
?Và°´@w? ò•âr?Òþç,r+?Zå!÷.qÄ?Vz*¶È?ï¥)˜ˆU,?ƒ+ò ¾ h?shîà¸7?pÈ¥f§Œö?zDæRqŸ?~TßßÝÎb?ï1¢ñ(?'yÎ9<ÄM?ƒ ~£ê˜t?p;«‡lÃ:?•‰Œj¸ÙÆ?{öºü$²?ï(äÙÞÙ?î'‡Æt?\~®•íc?byrX÷6?™5Ø}OÏ?6B9éä=?ïúQ$ŠÎÑ?<™¥ã»X?ÏR|ù?Ì¢Ö—H?CÁƒC®Ÿ…?:à¾JæìË?ïàjêÀ¹Õ?iÑéb¶Ú?\à腶rù?X¨Ë!PW?a$ ÕïQ"?bû"Vß?ï'Æž+ñî?pæ^‰oJQ?vË7n$τ?bpÂîy0?ƒè¼³¢HÞ?gzôûɞ?ïÓÂùþøÞ?dëqª÷?S¤UôÏ?HZ¡põÇ??q[^Ï/ú?aé;,xÇNAGN3FGL J1534.4+5323@U`7ßÕ¾
@IE`\a*À:׺nü7À<!x#'L¿Ý•VpqyŒ@uuœ9\?ÿZÞ°t|¿í9"ZÌf¿­š"i´¿ÐIÀ	è-ž¿ãŽ…ÎØâýAGNbll?ïö «å)C?O·i"ò?Fúp†ÙV?K"[º[#?=d°3 m?4L
"'Àm?ï}í6Ï ?ŒJ'U£X?}/ÅÒöõ"?{†I4ñ1-?'!áÓqg?…\çDnÛ/?îúû÷\ÃO?‹WkA""+?F
GÎî?‡…É
Ó÷?Zv̘¨?vÚifÜe?ï{€Yà#Ê?ƒU2ïcù?t簄hï?q‰îP·á?‡õ°dÄø?~© -ä?ïüúN³?2o…¢$j?)Ôß©xý?*1f¸Ç`j?3º_L¿?%¼S·¦?ïÚ³nUQ?jÊUCìMx?b-]ã¸Z%?_ú?´é[Å?c³qµ?a
˜*+i?ïw÷Œ$LL?y_w¸‰ûí?'o–m?v–X¨×ßÙ?€òš'd4"?a´‡¡¢?ïãì'8L"?[DͼÅCp?XwìîNÖi?I7–Òøñ
?_®ð¿Uuê?S€§LÞSAGN3FGL J1534.5+0128@´‡ßÝË£@E¢¿ÖDEÀ9r´€ÈÀ;9oV•¿÷RH¿·e‡@ä8¤6V@:Ä@]׿çõ*åd{Þ¿ê%…sÌοã2¶¨ö¿ïÿÂáo#ØAGNfsrq?ïý:O·?8)qkIV?J¶vMÛ9?Èx*ÆT?3†(B-¶?7ŠûqYÍ?ï´¥˜Í¹(?ÑG'üþ?oІ'½Wf?p͚ô«Â ?uÄð•ô?{X'ßÕ?îï!Á¤XB?´<X$?ŽèEOõž™?}I¯/[?'§¥ 
Œv?‡¹X0*°§?ï¾÷\:"?|ŒÞÓLJ??dË龑?G}AëD@Ì?~"&tq3¤?{Ò#öµ?ïþŽ‹ý|?!?ݙ¦t?	­ÊÒÇ!I?:ãyùC@? «ÍVDïù?&¸MÔ¦?ï䈍­¨?fÇLD¦?Y–þÎkw6?TêµÆ?]W呌&a?_I݇\?ïQœ¡¥›t?"¤Ûiº-?ˆ……Aq/?s<48iÇ{?ƒ"R»?wøM"¶?ïóôÖG?Uã»'")Ù?
<t€$Þã?Á7UCΚ?W,p&¨¾)?U½™HÓèÒAGN3FGL J1535.0+3721@N: þ¡@K.ßç[ÄÀ:kc%iFÀ;èa'ÑÖø¿×IñàO@UáŒR3@é¾ RÔ?¦:A^2ÿö¿ä0+Y¨›s¿è¨ærT+?°+n"ï¼AGNbll?ïáZÿ¼?hÕã.]•?V]ä'U†$?Z.Òâδ^?cvQ2ìÌ?`üNŠÉ'q?ïµ
­–¸?'¤ð@}?nÀø¿Ý?r!<rÅlù?vö/Âqq?{Ãœ€øc?î^©â£4?˜GnzKa?›°Ò|Vk0?Ý]»2u½?˜yñ*©Ì?…æFB?ïbÁ>µX£?ÇtÀ"¥Ü?^xeRN[J?jà=Ó¯Cí?'ÀQÐhsî?wuÿÌف?ïôðꅼº?R=w¡K‰?A^bµã&?DAÒÝrNÒ?JÝóKZc¹?HºÙ´Ó?ïá—ÇSÞq?mÈ"xbض?\²×l•?b±Ê¤ζ?`Ì´¬³?_Û²¢ºä?ïDÆ%
Gú?'ýT¼Óh?Š<ŒÎ/#?|çû6è?"¶:)Àšo?pqFÇk5?ïìkN¾»"?cîr·?1:~Xíˆê?1['ãçí?ama¶ãV?b³¥.ƒvAGN3FGL J1535.7+3920@O«"?½…1@Jó®ñðÀ:§ouÙ ñÀ<bfýe?Ý©¥wÀ£@@d•Xí,@Ë.@/E?ïþ¼I$"½¿Ý³"ê÷Á¿ç>Ԁd-@¿ßÓÜW>ÅAGNbll?ï%R¯û/â?À–ºìû?•'w˜[äª?ÀvKòØá?x¸É½Õ4d?‹"qƒÔJ?ïW_#so?›>Tø }H?"m̓MÆ?'öŸÇ­à?…Ì
fX?'!p1#5%?î:/ó|}Ä?™Á'µÎ? u'ÒàjÂ?•g$û'¯Ø?—ϱãÐ:?…‹sèºQ?íÍÔm?­rŒ:e |?©v¹r
?£èãþžR?¥oœmyú?¤w²ÞÌð?ï¤ø†É?ÃãeØ|Æ?›fw0Í£?Ã鏃ɬ:?^NœF¥\m?wµxfPéh?ïËMÅa?|7¡}ÐÒ¡?há¾^eŠ?m¥®
6¤Î?kÐ|¶0<'?sÚö™l}£?ïé0/ț?'J¸£¬†?'Š¶>ûD?‹t0–…Cõ?‰ÒžvaÖì? .ÒÝÿ@?ïwgÄÏB?‰¯+!"ß?"ã"é+&?w¿Ë¹O¸?z…Ôø¤?'d­Ž\AGN3FGL J1536.3-4949@tƒ!_Ìr@ Þý';À7)&p­À:"&êþ@&»¶Où@y6R!Šê?ù×2
ï+ò¿Ù+¹öËпÜh‡#±q8¿àKª7m÷Í¿é=ORòPSRpsr?½¹¡:¼ƒB?¶¿Ä_A¹F?ØzRAt?Í|–€¬Û?ࢸ§%ô?Î{/'y—?pçE°Î"?|jm—«?çr鉅5?Ɗ+¦›‹?ÐÙ­QB£û?Æ_IDJ:i?ÏQCË»¢?²;æÇ0û?Ò â^ë"?´ú9¥§¿®?Þ6|.ž,?»D˜'º§S?›ÛZ
¥u"?,î†[R?æPuŽL‰?¶,Ÿ¥Š?Ñ©t$Œt?´ÿ'H'"?Æúß.Ï d?Áðžì?Þô4 ½?͗ûî½&U?Վ[È}²³?̛è؊ßÜ?|::"Ò_x?†²".©2?é÷Tþ4"ò?½+9)AlÝ?Ç@Ú4X;?¼Óú°Ï…?ÒþM‡a!?±)é(¨3É?×&a»SJ!?²ãÖÂñŒ?ÕÛP½K"B?µQvôá¢?¢N+aK­?Œ67µÔÖ?èáâM	ž?§˜ÄÁíI?ÇòcA:T\?¥Ðä*(ËæMIXED3FGL J1536.6+8331@]z÷@?åğס<À:~†TBwÀ;ýF†Í;¿ì°ç¶Tˆ@ìF±c@ÙH@`˜F¿âD÷\݇¿çð›nª¿æboð9Á¿àâf¾O%AGNbcu?ïßÜyÇ?lh
Õ0–œ?K•,t	?GCæÁSÈ?j¤Y| J?jQH\¼Ï?ïdžÞ…?ž˜	PՓA?'õ=áºS?'$¹ÓêÔ?"ÆS!jQæ?'‡tËPmM?íÌ_ž•5?•@-)ŸYÏ?•ïwò§?ùZô<-P?¨B?«ì¡a?oæXô?îàésî܏?'ˆfªÿ©‹?p$g9´O}?m¢×'¾
Ù?ŸÙ·¼¦VD?'"<[t?ïö#Ëa<Ü?NI†z?2¢çh—?/…H¥@Œ?N(ùjj?Kj¶c?ïÔ4	>dŒ?yR+.I™ó?c\TÏÆ}?fçÍ'ú?ho¡Ù1"?q+¯°ÛS?ï,ÊI ï
?ì´Ï (Z?"4Ñîr­?mE©+¾Õ?fœ\»™~?wWÍì{4?ï֌€ENƒ?eLiõmÿ?EÕWWX?:f	ô<¡î?qÿä»Æ]?d1mÆ
 AGN3FGL J1537.8-8000@s_<`ŸÀ3}_²?À9CÖNUÎiÀ;~æ"ôï+?Ö!ª°ÔYð@KÚsÿV@}Ç/$Ü¿á¹SK~ó¿ãgâ(Ý"¿àRÁՑ±2¿çœì='AGNbcu?ïóö,?Yû×^,¥?!ízÙ¬í?UðLíIÑ?W­æI¡çÍ?YJË­In?îÔ[Åß®ã?£NO-å–r?'•ÒÑOé¤?}Ö7²±\?œ)Þ!ÞÍ?¡Çaºñ]D?ï
›-(¾K?†"SðÜ»?…çñĽ…?t`ë!&Ž[?"$¦`N	Ó? »ÔY?íÕÖoI??–…e¿~Xì?€Op1ìŽ@?qÐÑ˃†f?®Ž¼þšò'?•OöÜl‡P?ïó^c…ÿ?Š)iézBì??03É6?rɼoÝ?Q€m7`Ëd?yH±Ǫ?ï¤ewÓ÷?‡×‡§-õ¿?iûÕq[?cFB ^½Ï?€¤ãB½¼O?"¼j➆˜?ï så¢S?rnêjSÈ4?r¢þŸé!?]›Kú6ž?}#–|sæ?pZeÜÓå?ïo˜6B1S?wd'…̦k?px$:?T5ßF2Oš?Œ¶VŒÖG?uξ¸æ§œAGN3FGL J1539.5+2746@Eôv?ø="@Jqÿ΁ÙÀ9O~Rì6À;šÌÜ­?é(·²ù@Ésô–$@©:ÿZh¬¿Ílï)÷}Ù¿à¡_ðÚÕ¿à›Ôÿ˜ž¿æmá|S°AGNfsrq?ïþ
Añ`?"<Tã*È?˜4z?d›ÃËð?™I0!ˆm?+^<"?ï¹­H«ž?€Öè˜|‹?n—éáªå?sisŠ[ü?sÝfƳ+/?uÙ‹1?ïa°Ïô¨?'m—+Vû!?ÊŸ-ÔºÝ?wU½ŠP®?…É,Ö¹ô?y1ÜúÌúA?ïӑˆ0Ä!?vèa
®p?Jec›ÎÓ?QÊ?0Æâ?rçO$€^?u¬0K‹Î?ïþÃ*É?ØŠ#¬?³
ˆú?‹\뗁?çš]ŠŽ²?Ç:&øÄ?ïæWûk?gï"3>"è?V•ƒý&?T*WÏm9?]Q́ð[û?a°œFÈhp?ï¡´*òûh?y$¬`ßQ~?w þ9ð©X?ppÀúáþý?xìGÂ.Š?s+åªËL?ïö¸C±cB?P^ÕÏĤH?<N_w?4œ¸N#›?Gn®Ø+r?K"x7Á,ÇAGN3FGL J1539.8-1128@v2ï€Uûµ@@çk b
·À9ò¬U^fÀ;s×gZ'¿µc9ìLÿ>@
°R°Ñïv@­Ó %¤Õ¿êȆ)þ¿äj©…䠿ݨ"õèF¿äé£Rˆ–›AGNbcu?ï"7Ñí6é?ˆÚÁõ0ض?_±íÄXOó?Y,…DÒÙ?‡;ͽ`é½?†ä|Pdo·?ïD›.³á]?™xohȵI?…›•A|>?ˆŸ¸<}üÞ?‰>½Æ,q?'úê`iHÚ?îXÄ]<œ?•>Ó0è1?iÎßòZ?š2R,š?¢IÌ­¼=?ä²~S?쁏ŠÕ?¢uÎX% š?Š;‹¡ÌS?€Ü;ë>®?¸¬ŸÐë??¡W7èWJr?ï飾qÑe?w¢›¨Áðp?CçáRü3e?Tr3é"p?abIgzR?rƐ™Nö?ïĸ¦Ð
õ?zÆ¿w8Ã?jy¦÷?f}b»
î?pŸïÙ+¬?uhw?¬G?ïkêU/¬?yb\ݤ?}fXâ·Ë)?jQ§S÷½?†R>6'¡ˆ?r
ßÆì?îó="¶
?'·:Ý?|2¥ÕMq?dÿ*`Z?š‹£ú«U?€b®`OôAGN3FGL J1540.1+8155@]—¿¤Æ@@{¢ò(§À9‹QÿÅHÀ;}êXÎÎ?êú"9!@T6
-?ù¢ºÀèG?ïøœÀ¯K÷?£B†jñC,¿ÛèQHÙ¿°wËNٓAGNbll?ïÓDX¨f?sÂ'd^ƒ?p"êÈ.,?pøF~¿›?W'ˆ¥z«?XÝZ!?ïlÐ6f?™[Ï)`†?€Ç!z»u?‹î*Šþ?"ÝüPb?'õßY†ÿ?îeÅ'»?–y<‰û ?›Ëzô/?È?æ}'»?—{áÞèêK?‡¹W¿?툙³.4?§qó(ÕV÷?"DÜ?–®øØdþ?­ÔbD"+¿?¤uÌLlÐ?ïì=Pš{?[\–˜+/,?\ͅŒJìW?UƒMeç?Eo´^«pC?@Âuþɵ_?ïʽ«œ¦i?Ê1±	«?gY@ÿÈ?n(K§¶üK?mé0¾Ï?wÈjZlî?ï/"k'/?‰^ÍÎ|Ë?ŒÀtR8S?ƒƒu (ž?‡Z±'6?|çE)?ïP|%%º‹?‹›°cú??šFJ6¹á?y\LryŽ?ŒӗMVM?…fÄ ©9AGN3FGL J1540.8+1449@8`Ÿþ7©@Hhâ:¸cÀ:œU5¼À;xÔu§L¿°Çñm<°@DYgzb@ÂgŸÌc›¿áè+ðɬ1¿çPÐò@T¿éØi€¶}¿ª­eÌô¡AGNbll?ïÙáö{?voåtÈ+¹?WZÞFì~?[
È-idZ?jž:ž"ž?r|,ßy¨.?﬩ô°–‹?…Zá®ùV?pÉô"Úϯ?s;G*î4‹?xá1fŽ"?€Qø`RÙ?îY[Ö?"ßq4ã›ø?"Öæ¬ý7?†•·^fî?Ÿý¶ù¦­?Šˆœ/ñÁ@?î¿Nh³?˜ƒ¨Ÿ#¤Ó?g˜Še ?qwˆòOÒ?¢–uc3Ÿø?—ßúڄÎå?ïõq"øÀ?XqÐ0;Rƒ?;tH'Äã?>pÓ1"‹?L‹5ÅD¹?St¥\Þ	Û?ïãþòä¹~?fsˆlÜ[e?YBªJô÷`?Ur'Ž¦€?^¿pj	¬Ò?`B¯g¸&G?ïZb×»"??|­/A™Ïá?'¬‹^Lwa?qgV
;r?†º¾»
Èñ?s7ÌZ™!!?ïƐ—´´u?pkªFÏX?H¡Be¼?G½yPy¼f?y£‹Î"k?oMäðF,íAGN3FGL J1541.8+1105@3Š"€,á
@Gw±ÿÁìŸÀ9ÊÂñ·üÀ;§À)P[b¿È`®Å›@P‹RY@Þ1àwÏo¿ç>O"ùÝã¿ç
dHI…¿êÛí›=L€¿ïþÉ|w±AGNfsrq?ïÚ÷ 
!?q–R_Æ֓?fXÀ߁ü?e.I±á§?]`¦´6_W?j0, M?î¹èàdëM?¤TîQ©VU?•0àƒÊ
·?•­"ŸË*?"'qPY?ž¢•Ã¡?î6¤+îÆG?"úh4žw?žoöß:¦?‰'Ú(o?š¼\"ßu?ˆ<Ô•?ëÒñ£´?¬Þ´W•P$?²i"Ô!r?¨*ÈáŠÛ?­þ¨¯9¨"? #¡ È8É?ï«c@Ê©?µ=Â¹œ›?_"Ê
"-?\pRI<§?4–~"×ÿ?µF?1F³"? ñ^Ÿ?"ü~SÏÉ?xígÄÎ8?yÈވÇ?u¹‡Õ/ʃ?w0žÐZ‹ë?ï	ó'™:é?ƒTЖ¢Å›?"#bR'ª?|ÒajŠÙ©?‡<q|Bfo?r"‹¾Ó¬?ï@½9Üœ?…-÷&k
?…ÞnU‹1S?xWuwI?‰òC='=Í?€'ß*eäAGN3FGL J1542.9+6129@WØØÀ  @F²`œ˜RÀ7Óû-2h2À:ì³Z§?óòÈê•	½@~b«0E?ýKê"_¿Üؼ'@¿@¿ßû)ñëë¿ßJ:-DÔ¿â½'{Æ}†AGNbll?ïùÙk€,?@ºïù"É?,ûÞ©Uˆó?+
rB¸Ç?A\Š¼¯×?9¤Ãp-?ïºu÷"?€"Y{iä?n_߅¬h?nCpþ$õŒ?sñ…'¢?wxÇI"±L?ï,kð,?í1î¥êª?‡Ql·ÁÖW?"wÐí´i?¬¸"Ž ?†Uçïç#Ó?ïˆÓؕê?‹Âqmð7O?S¢Y³±çÿ?_à5ö'?‹†¿Í4üŒ?‹ÄsÂ,?ïü'ßC¥z?6ÕnæÎd×?%¬±†]Æ?)G´rˆq?0š¬–sPF?(À¿ÌxÛ?ïãǕ€ZX?fLJ6R<?XnèÕ2¡?TÄJ¹¶ìM?`fwý>d?`Ò¥‰§Á?ïyâÞËÁ¤?ƒ†F‡,å?}Ù0•l‹á?xˆˆÑ%œ$?'š°·é?|xI
u>ˆ?ïßðZg÷Ø?g©K€Ãr?MËé]1J"?Fœmçÿ/Á?hœ«C{"û?e,ÂU €AGN3FGL J1542.9-5141@t~œ…×E@Hm`€žKÀ8Œ7ùk'IÀ:­AÞËÓ?êaV8¾.ò@
h•»=®6@èMß[ð—¿átŠô¿èÝ(œx¾z¿äˆJYj{¿íÒç‹BûPSRPSR?Ä®14¯Ï?¾èZ:Öb?ÑkSžkC#?Ç&Jv{K?âÉ̽2{?ÊÊäräVµ?³rÜÀó–3?¼"ὅî'?Ô®™¤è?›HŸšÔF?ã'ÍY†üU?Èm-ˆ÷Å?ÑQڛÊÿÌ?²ÜX-"Ñ?ÊàrÉ­é?¯Ïÿem›?àžõÿԔ ?¸1š)"?Âd§Ùg(È?§·­êM}?Ñ÷#.10?¯Í«Î]B<?âkD†6?´`÷øBÉ?ÔȧOJý?Éõû‹?ÔÑ9ή?ÈxÓyAèá?×"•{4C?ɹŠ€k~?Ðm"<ëó?͞ßå¿s.?Ó¯Ó"&q?½ÇâAÔ
Ú?ÛãÐïòÝ?É\|Ù?á—â›|Y?²&šW0rÌ?ÆO¾hIÚ-?¦i¼EæË?ÒÆñ¤7?°Ä@Yˆó´?ÑâÇyÀz?± ‹J¹q?ÑζÕGMO?§è·_¹_C?Ý,fc>ò7?°r	ke^MIXED3FGL J1543.5+0451@(|ȵ1¦@E²NŸ CØÀ:,ÅÜÃkÀ; 	Å{Ÿ´¿õºD²6žx@
¸TûÛ?ÿÁàþ¿ëL "ö¿Û±WšŠt'¿âTÃRß̿ĸÞAGNbcu?ïñûقµ?Tíç}hè¢?;'†«a<@?4©P&™S?U%0îŒÉ}?RZ 	H|?ï·ç1æ`?'s-ä/»?oŠÉ¨n3?rk÷¶äØ?t…""È?xûá¬ê™?îïîB˜?†—tØy?‡³K…r?t}2G¨?–(¼NøB?'.ƒ{>?ï¨íZ>˜u?|Ä®Ó5Y?#"o­ak±?(Faù\¢²?…x·°yé?|˜º²ª?ïúhsÜƕ?:‡e:À´?(—$Ð t?3¶{?@8h(#lt?7gœâßÍ?ïçG×|u"?d¨F"¾°V?UÉlµÕÎJ?R{H…àÁ*?[¦ä†Ú{?\Þ¬=I-d?ï…M]ðä?s<õ1x{š?yaö…iÝ?i¸e‰â	}?û­sŠÎ?hVlÝ¿?ïðÚü…"?Nõ§Øˆý>?íㄑTò>ùš‹í‡,?]º˜"üCå?NÁÕBÍ]KAGN3FGL J1544.0+4938@S̸`.>@IŒÕ£5À:Zäd™ÍÀ<åB¿Ã}}!éµ@'‰¹QÅÅ@j¨_°ٿ׻ϣZ§Z¿àe-Qzy¡¿ëòÀb—`¿Ã‡­,@ŠPSRPSR?ïÛjw ©?°÷XøN?\$†:‡?o0p8¶Ð˜?fNö+lŸ£?tMqN¬?ïÑÍo%
?{"u¿p«?_xwÓ{³š?kž{™gi?n€6yÂAa?tðãè}C?4³2i?'ßÓÊï?ŒôŸÀh¦?€JPaØ:?š3Ɇb‡?‹r74\™'?ïrb{[?RÙ¹Ϩ?bÔ\YæYõ?l)_!´ã?Ž²J€YÅ?ŒjõÚF¹Ì?ïi`ì©â?Á"¥ 'v?€^Ñôa?£uwå僚?—R¤|Fƒ?»"Esҋ?ïëäF¸n?e@Zà4¬Z?M£Ä¶GÀâ?Pñå6ÛFS?Yf*ïr·?^v‹d6?ïW«OÏv?ƒC^ [—?ƒ|ý:(Ÿ?y«/ ®ð?‡¯P	ƒ?|8։,Å¡?ïëÎf™«Ò?f_"6f\–?=~CB À??ë؊«ú?`Ñƒz?cظ¹}ŽCAGN3FGL J1546.0+0818@0ÄßVø4@FWM@$³>À9°åÜhKCÀ;`üÀ°^Ø?äfIyà[@šÁq¹?û
i€L@ ?ïî
ñº[Ë?çJü©š~Ø¿×XŠå:›¡¿Ö<]ÍÕOAAGNbll?ïû<ÕÚxÃ??Ðü <¢?5gQ– =ì?1Q9Ì[µ?0±ýŒn…¥?7V0¾zûõ?ïZê/ÅP¾?˜¦zÚe'?ƒFÛðÄ,?‡ìœ=;^v?…þ˜æ…|?'Û×–²?ï$‰ˆe¥Ý?Ý#Á'8?ˆOTÕY;?"÷iμ?ŽŽI­i?"h–3_P?íZb]S~?­ï×ÖЎ?©:gå)€{?¥@Ë»Œ±?¦ñö¹œ?¢Ã)œòÄ¢?ïÞã®CRn?­Gø%
éx?bÔW={!? Ù´Œ› ±?\õ=²?˜Þ"NxLÝ?ïøµ®x?'šxÙ?kŒ·hÝE?tà"qÃ?p]ð^Áé.?z¯±îhé?ï.ât1‰?†|àσÎf?€EÓg|V?€¡#©ºèa?€2†õ…?}ö?ÒEå?ï4«À…
=?‰Þþ\úd?Šxó~3Ùï?xøÚh2Á?ˆ\RÊfç?"³Š`•AGN3FGL J1546.6+1812@=í2ÿ0Í'@Hg¥€W©4À:Gç.wâÀ;»Ä4wÖÑ¿Õ¼ùßÄ:@
Yžk˜y@gnåhz¿ãÉÿ&
}¿çf¤¢"È'¿ÐoXÞša¿Þ~K¸˜ÀßAGNbll?ïÜYrÀšm?oBSˆ"ƒÐ?B½äØ16»?=©¦ÈÀ¸?n÷ÕòPÅ?màwÄE¶?ïªý?cö¨?"˜†I/ÉÇ?sÍ•uqî?~˜ü™Kɋ?v´M˜Bæ1?yIˆ2á£!?îLtÝÍ{?"|ù†ÜV?'Ák8ÀãK?'ÀÚ9=¬'?¢Wü'|Yˆ?žU¯Ï?ï$	÷Œ?ŠÓæY~'?^d"¤íó'?`A'#ˆ
E?™˜xÛ~®k?‰¡œ°?ò`?ïö ªçÂ?S±sªÒ8?0ã¹|5[Ä?1ý•²++?Ox=XB
?Rqç‰?ïâ!t]¹³?g‹§Š²?[«Öç9«ä?YTp'ÙÛx?` U%?_y"f–fÑ?ï]2¥ï"K?|¹««"–Ä?¼;ò¬ÕÀ?q\tEZQ?ˆÕ8†MDS?r'±î¦?ïÕÅ:Ã\?cfšü3¯g?NΏçwå?>$R%)ðÀ?qœËbÌvc?aáŠI¤lAGN3FGL J1547.1-2801@u|€àe0@4•2Ÿ|àÀ:MÎ_ªÀ;ƒcÎÜq…?ë'éýÎç@
üF£ÓYY?ûRÄá
x¿ïÍ3Ó¨Dh?ïø5£®h¿á&¸ê¨æû¿ÝG:SZgwAGNbcu?ïÒSWüýR?t
-×}ü—?bßhòdo?d»nÕ˜|?jÍ>à"r?h6ŒßŸ?î6<ã"ÁF?²^P꿁?›_‹x;ƒ?š§µûŸÕ?ØØt$´?¬˜àž&Kb?íÁ¼»3ó?Ÿ`ŸøºX¯?¢ÏN¾FP?"ü"Oá×?¡Èo´²"?çRü¬W?éøû i¤?»áÝ!¦k?ÅÄèk¨‰e?º{ÃVX?¨¼Î™Sï.?¦¹Õ>Ú]?ïâNv°‹y?jƒ̝?Z<
"MëH?]]Ö0ã÷†?`"ƒÒsZ	?]€y´5J?ïhw{j74?›òæØ_Ô±?5Ӟ½Ç?ƒ'Ê@èí?"¬M'³e*?•ÌÒF­?ïɳ?GÞ­×?´:÷Ñ
?"Ú«ëR_N?ŽeCc'^?~tÇõÆïÕ?íd¯Èb¸e?Ÿ€£Ï$?°×P\A}?›ïq߸¯+?Å}{•r?…`aSQîAGN3FGL J1548.8-2250@u½¥¶™…@8*% Jù#À9|©žÊ[À;?fg=%û¿Ùà Fåu@'#C¦óÊ@b#¿ø¨ô¿ÙûºÁ1Ž¿äcíÖÝ?¿â¾ŽIj"X¿Õôg25©§AGNbll?ïßheUV?i$)¸ª?S;ԘyX8?L;dW'ÂÙ?gZ­•¶?dèQÙØ¡1?ï~èÜ,w?–Í—jBӊ?yõCžóC,?"pônXK'?ƒKZ)ì€?'°p¿"zÝ?îtOK}èõ?–s¬¡¾i?"GR=Ô:Ä?‰%pÛgøÀ?.ÄMG<?ŽgÍÈ?ìÛÛ=Rñ¿?¡9H×ú?mÍš¡÷J?kñ»ÜîÆ?¸2½‡(‹Œ?¡1¬m®D§?ïô…‹Î2†?Tã†ô?BŽæjò¿›?>HÿwÍä?KZ껸?Nñ¼Þ7v?ïÔÔ'ßíç?w«ãs,rz?as\A
?Y<÷¢'?i¸|±'.?s‹×6³7?ï`äÈROê?€ÜêŸñ†?'剚
«ç?wŽê •*Û?"áD]dû{?ry¦Q¾Y²?ï,ë8¦BR?€Øå~.b?T9I
"	?Dã©~b?™N¯•£?€•æv4_AGN3FGL J1549.0+6309@X9Àgn@EùJ?¿2°À:iêÝYÀ<‹?cÃÀ8‡Q˜y@›@"Yò@Î8£NN¿æ@Ç/ÿÌÿ¿ìpژ½P®¿ÔùT~¡4‡¿èƒdç"AGNbcu?ïðw'©¤:?`€#n§Ñ?7«"†5÷ã?@"ÜB®è-?Y&2ne,
?^q-ò.?ïˆô±JîÄ?¢wví½Ë7?¥Æ–Ü^¾?¡9<Áå-»?{ßàË;c?ƒv'@º?íÑsû¹?–"­T3k?'£æ{Sñ4?'JԔ¶=¼?©–Ü'¥ËÒ?'"qd´D?ï{/`é?ˆ"©8H¡?;}Ú?"?FÇIvªU?#œ¼år?ˆ@Uði4?ï÷¡¡@?N{ÐWu"?-¾ýœµà•?0/ã=?J	¹´6"é?KÖYõ²&?ïÚ}	@¢?{ÿq£P
Ÿ?a‹3	ª"?oˆ:ˆÔZÏ?c÷î–z›?o‰´¾rõÌ?ï
J¨¶ø?‡¥¤&ÖÓ?ƒ¶'#š`×?wáX2¹ô?"{—h ©?ÿ*‡.U?ïìÙ·cP?\‹€x©?ŠF\ðu?h¯ì­H?b¸—þ•?[ÆÄëk'AGN3FGL J1549.1-5347c@tuè_ÐJ0?Û¨h r2ÅÀ7p@Õ³%\À9ý"'¤?ò1˜Ä1²@ŽG…z©@xǟfb5¿ä̬¶¬Ï׿èD®?îØe¿æïçCp˜¿ïïå|OTHERsppa?‡¬«äÄ<?ƒ×æ !aé?ÓZJXœW?ÉԞV±\?åôE+z¤ƒ?Ê"¦¯pŠ?gÆ3k=kë?ÓaGŠÜ|?ݲLx©‰ý?Ãa±MîÃ?ᐢòU?Ãrç¸$bû?¸\˜f¦™?¡ß¬•£)‹?Ö¢ut»¸?·*c?þ8N?យ²‡ëá?¶Î'•Ét`?¤q¯àKè]?š,uB¼?ÓóÑÔ¤?»®"i›?ä¾üú-ê?½z¾?ÉÍ?{DHÔº?|ü*ŒáDg?Û"_Ð9Ã?ÐU÷¶·?â8Çû4qÕ?ÐW?ÊùÁ€?|¯><=ØZ?Œÿàx~«?àß»ÙNT;?¹}¸ƒi¬?ÝÍËTҕ9?º–§T¬ø?Áú2¿šà?§yÝF}È?×"AÉN2?µ~ÃÉP½ô?ßà¼R ^?µ"»½L?¯$Óñ™Ð?£ûh~ŠÈ?Ñúðç^H‹?³Õ±ü%¦?å:[Â?¶¤,SFÙ@MIXED3FGL J1549.4+0237@%¸çÖyõ@DtÈßØBLÀ8j™ç2«À;UýgŸKŠ?ÛÑ^$@ÑIOL@´é •vÊ¿å;ßÊÞ鎿æGkX,€«¿åÉ_›'8:¿ë:ui0AGNfsrq?ïø¾&Z¡{?Bä½Bîª[?B¸ÒÈýóÖ?<‡¦l0Ï?4)lCÚ?/ÅËìÛ¥/?ï¥Rr=µ?Œµ8Ìô;±?sÓ4U':á?ƒš«c¯ËŠ?yƒ't á˜?€M4DZ†?ïN
¾¹¨?…Tþê>=L?ߞCt?Údz©ðy?‹b~qÂ\?yQK;Â?ïoK
Oý?‰téÓ¶?fÀ…ºÁ;Ý?cæ&°?Ž}Úé¬?‡ï%z(‰8?ïûô®ã?2R;ŽîvÑ?7áw«!+Ý?.
Bq)‡2? ò-ŒHP?ÌbZ²<>?ïÜ.[7‰?j°½"o?`$¶ÈÈi?W×]îÌg©?c­;:}?b]"ЛF?ïtþÉbú?uµ±ë­]?€ëöVí¥?lï@¢*	…?}ndŸ'_î?lý ˆç?ïä¹ù
˜_?e›)CG¶Ï?Jµ¦À¥–?AÇ8lr?d˜®ÍN?d*…ƒšÑ=AGN3FGL J1549.5+1709@<ҏÃæ@Gç
€CRÀ:–ŠQýù–À;ג'µP¯¿âjڋə´@f÷ºâ±?þ¨›ÿÊ{¿ë;iå™CÖ¿ÙS'Bï$!¿àü¦Mÿ^½¿È´q'¥šÀAGNbcu?ïûÔÃwt½?8#Œ5{·"?(Þà\s(?"¾Â6ý
?4êr{W¡ö?2nÞ¬÷¹?ï½|óE²g?~ûX,½$p?kÄíðß×¼?oMFöñx?s_i†T¹?vr)!S?ïTåw5
?ƒé'÷Ý%n?€É
W…è­?teŸ4lÒê?‰ý"Ð8‡?¥r¶ÿ-?ïÙ.H×y?j߉Î¦)?&FFŒn,?,«=í¥?r¸YgkDU?j‡º3Äô?ïþ±0þ¿?0؁Eæèp?†:ëŸu?'%%œ©Ò?"›§¸Ž?,㶀RžO?ïé7©Û?b˜cü6Ae?T'ö5?PøÊ/4'?YÑÌ÷¤»?YE—'7×?ï¨Q{?wm8sT,?tzز·äe?q$¾ïs#¼?wxœŽM^?pIP¸H–%?ïù å_¸?AU K'b?
l€Ì-N?óœM+?G¥¡`$o3?@ ¤µ5AGN3FGL J1549.7-0658?ó˜OÌû@A¾ß¤?æÀ9;´L£FÂÀ;DD<oò׿î求÷õ"@ëUN.?þÇÑ`w‰¿ËðzÑØO¿àkI]ǟ¿â¨ëy5K¿ÌØ¢cÒ§AGNbcu?ïÓ0ô6±?­>ȖöëÉ?qÑñø\ž?­EöҁX	?RYüìj_?Kž±ð²Ô"?ï­ëJD?"ÒÇV£ø.?qÓå4k?oój*ù e?xeyêBM?€à˜ÜÝGŽ?îÊ(ÕX®å?w)‡VÙ¨?'¶ÊÿX•a?‡ëgZD?"N²V?ƒö•t!45?îš/7"Û‰?•X-mÀZ ?I±}Ñü˜ó?PèG8Žò?¥öF•ð¼?•9ä%¤—^?îº?
~e-?ȨäǑÇ?¤)ی&k.?È«f†ØÝã?9ͯö-?4«Â1Üz¤?ïàï¤Æ¦÷?gÞ­[€¡Ö?ZQ€1?SҒ
x*?aϲ¤:Y?b>;Â~`G?ïiׇïUÁ?‡
+˜+P?")r.	—?~‡†`h?€ùô£'‡ù?kWóíZ.r?ï¬"?qíôÙ!?("é…ù¢'? #…W^.?"—eçÚR?q㣕QN'AGN3FGL J1550.3+7409@[8_á'p@B×@&`½À:oË
Tí˜À<¶ŸcÝö?á‹b¡àºë@¬P¥^ô­@›@bƟ¿æz\q½T¿î1=#:Üd?·ß¿¥"F¿ãìüÝAGNbcu?ïþ.(SӉ?0$<bæ†(?›"Jñé˜?#þtêòòÖ? O³¸–? €'º<ß?ï˜\ ?…OqŒƒ?v÷lúÿa?t~*rG?|ڐF—
­?~ÒCŒ O ?ïÜ$Ðç0?˜¥¯¥À1?¸§ÞÏ+h?}ÂFvþô?–ˆ'vÿuG?Š–Êïù?ï£oW7?ŠŒëHSyü?Z•þߍ||?h0ÚêM
?ƒì¤^f¹-?ˆÐEõz
?ïþÓ³×ï|?#"h?S!`º¡?	Æà×.ØÉ?_ð—ÃϨ?9ШЩ8?ïÙR±þ•G?m%#ú%ãy?b$ŒÑÝ÷M?[bþq:¨?dˆÁHIñÂ?eÒI¸T Ž?ïPåÛ3m?u€ä]?mðڛ³új?e'¼ó_?'%)Cëô"?Ž}œ"(Æ?ïë/t'w?g©£g¿?U¨°g=à?Tvéâ£v?SøûòYÅ2?`´€Ç°ï$AGN3FGL J1550.5+0526@,gÀ_A@EÜà@GÀ8à€If{_À;n"aKts?ílÂ|*¸@&wºL@¯ñ⢿Õ.J ã¿æáNö‡¿â$à"¿ïþÄö¶ørAGNfsrq?é#gó2Z?Â{E4UÅ?ÈúJ7Ëb-?ÂDm˜3èæ?"À¯êEN?™‰^?Ðu4Vì?Êl¢Yu€ú?䈩¤KÓ?Îo}nô2?»dÞKy?·ý÷ž#ð_?å"Ve"ª¶?´s"}B?Ï2ÏÏÐQ?±®i<2?¸²ç8"ä,?¢Ìdú®ñë?Ø.!Gð§?¹Kîs+>õ?Þ7VÙUœ??¿­//Üú?Ã`ö
Äæ5?±É'X"O?í
;\™ÖM?³o1_JGµ?µ"W6!îö?²²Ý¯R{h?€Öo&Ã' ?y§êaAÀ?ÙZÅFú?Ð<›gá þ?à±d#*?Ïþ;qg˜¸?µéʘñÒ?¬º
ؓ¸?éˆx4!Î?ª'¬'ù$4?ÃeÖ¼˜TÔ?¦Ó5坱µ?©æ툤ÁÐ?–®Á<׿?åé¹=_N?®Áa`wvõ?Ð(Z¬ý?¯—3È5a¬?°•©ÂS?u, ôŒMIXED3FGL J1551.1-5610@tae¿­)™¿ù­1@ê«ÛÀ9²`9ü{À:" z^jï?í·ºbM8S@Ë îؐ?ü ¢qON?ïwÌT×È©¿X3¬Äˆtr?‰7º£ÌŸ¿Öþ«OTHERspp?Ô¤þ^1?Ëtaƒ ½?ªæRŸ~Ú?©*,‰¬ÙÁ?ãÿÖ-Ú?ÍÅÁè˜/?Ñ/:жfY?ÒA€t?Ô?·îÿý¼?±Õ8?äˆD·êèl?Ñov¦ï)?á
­\O?·<JÌì}"?·ç«lÍ*7?£C‹êá3,?×ìÊËüÔ?·b¥©>ʍ?à±Eª%¥?Æ_‹3'ìâ?¤â,	ž9?§ÁßYC'?ÜH\ï³ñM?Ç"Ú
"Ø?ÚyÂÁ'Ÿy?ÏF_d-já?¥œe"?¤6^jQT?ákÞê3?Ðgzž½×?á3èhšÚH?ÖðÁÖqÌ?²L¿ðµ#'?«FBævÅn?Ùÿ2'H?Ô»¬'œ?èKo•E?³œÉ‰À@t?±OãèÂ?žw7¥ûÖ?ÇQГg?±6"¿'¼0?åûo¼?P?½ ´3+"?²ÈNs¤")?¢K -Õ£?Ñ3õƒ'ßv?¾JÿŸMIXED3FGL J1552.1+0852@2q_¾¬y@EÓ7GMœÀ9õäžz©êÀ;¯%v²?¦šXmjÁ´@ÿ-ªˆ)Z@®{`sˆ8?'`ÏÅòàT¿ßŠµâ5ÐÙ¿éñ¡À¯ˆ¿àé¡r¹–AGNbll?ïÎò :Õ`?}"¤Àr?uÃس#?{ÞXÁ/[H?L1a£²?I§¾€N?ïWËáóÙ	?VݺäJ ?'"÷)‰ê?Š¼†µd›ù?‡xR ›G?–aõÌ.?î''K!^?›l¶j=i ? MÆSÙ=k?•ù@í1Ñ?št¦RSy?Š† éãí?íTíE
?¤Î#àr?ž BéÕ3?—4WdYµ˜?«âeî1Ñ? Ý<eôÂ?ïíeÂOy?Ž¬>Þ¦?Q¥S‹Á2q?VƒDãÄv?S(jÌç?Ž}õ¬È~?ïÎõ!Ú"?yµ1ç5D?e²†þ@?d9¿·¹ð?kXW­'ƒú?t;@ÇÀ#i?ï.U‹Ö@?ŠœQkÙ³?FXòÃ?†	ó£ð|?"jäW™¡?v›ç&h=?ïw;'ô:Ð?ÔXHtś?vë+¯¼?dpŠ>KVù?†» &<?ù ¯üF2AGN3FGL J1552.9-5610@td•`"¥¿ü#pÀ\|À7'¨|‹kÙÀ:LÔ¯]Ÿ?Ö.]pžx§@}Ñ2¸$@@YŠ¿Ýw¨Ãƒ"	¿ãÎ6YXa¿âo¥ßøù|¿àŠÝâɹOTHERspp@?ÁA«\1À?Âރ"%ø?°Z­Q°Ý?¶‹þôü¼‹?é¤?•AEE?É;ƒ
æó?±xp™L"?¿Ê¤q—zŽ?Ë5n'ç¤?Â{ŽI?ç–Köƒ?Ç3š ³G?Çôá^)V?±ƒ›±ÝïE?½äÉÙ'y?¥ŒÇóž?æF.mP»Y?´C®{_1?ÀWµz£?±Iù
?´‰ìzj"í?­évóô¦R?éXÕZdi?¸ÿ±Ê&¥?ÆН/n?̺wòsó?¯dë‰rÒR?·UHEŽá?èU‰û¨¿?ÐÎ÷×3ûR?ÂðBþW^a?Èn•Ž5ý?Ët8¹&t*?Á﹔ib?äfá ‹]?ÊHÓ6&
?Õ50®žŽv?·¥
ãe?Á+F¢C)?§ª3¡–^?á–)gû?·z "?Ë WEXœ?ºXQÌa©$?±öÜb8?›Ó¼Pô?çéo‰"ƒ?½62Š…OTHER3FGL J1553.3-2421@u¸ÚŸ¾vÉ@6Z(Àª'À9YêPkR^À;WªÒ§a?éwØ?á[>@½¸Ûÿ@<_":4¿Ì[>¿çÓSà¸ù¿ào ½Ëä+¿î,º~t,ÖAGNfsrq?ïiºÙ°5?…—¨NTX?ƒîƃôÍ
?ƒþI[(É?bÛ*æb	?aAì—~?ìÚhÊLr?²o<5ÖÊ©?°+V+yO?¡wÙA¯Š¸?§‹­g"ª@?®J8§nø?ëwK5³k'?¨÷}Fh?»E	Uwx?¥˜§Æ"5?¢9£Ö,Ÿ?'÷*ÌåÔä?ç5˜ûäèM?­‹Êjp+ú?¼|À/…~°?§5Üô]?Äë;ø©Ÿv?¦|î²ãˆ?ï³»XRžÖ?'÷ĕñAj?€Kaœäçö?'§…dQ?V.Bn´å?Séa@T^r?îmóPD;? <ÀO»Õ?àOA-û?&"`Çw?"aFåï<÷?˜ƒ¨›´Ø?읎1ö6?£÷o€Éò…?µ©uÀoý? ü'"ø?•¨bÈË0?ŠW@Š‡ùv?ìtf•q}?"Gáí¥N?±ñ¢‰^6b?É¦×¹˜?ª…t‡\h?Žk¢ƒ?AGN3FGL J1553.5-3118@uieà.©a@15·?œÎÀ9…àãÛKÀ;Oûx±Â…?ø(0…ÙÉ5@>4r"‡>?"3/ë¹Á?éÇW±(Ó?ïû¡ék¶T¿ÓSM©oê8¿×æõU_¶}AGNbll?åim$y9°?ÎÇ÷+IR?ÀÁOÁsl?ÂP­*wx?ɘû­¥Ó?Í~#ø¾ÔM?ã0çÈýN?Ò·V"ï?ÑÍp¦†<?ÏUÝy°Y?¿C{S¢-?Átí_5çæ?â›ìy?¶A3yo¦®?ÑUSëÚL?²_à%G¢?Äý5ºõ…?²*6ôْJ?ܱÔڙ?ÅSý-<Ï?ÙLä¢?Å¢T£²ç?ÄÑÌ;‰?¾=SWÒ?å¥A3Á?Í{/Éú½ÿ?ÆDý³Ó	Z?ÇË1ȋ/Û?Ã%ý€ò"?Ææ¶UŌð?éI€Ð?Ïùs…6?Âãy¬¿;??Èå"o48?¯à¡@Ýè?¹$±æò†Ó?âç×IþPÓ?´³#jµ?Òlëär¹d?³TãFHÕ*?¿
–÷Ý?¨æ4abnÖ?ãh6»Ë??¼Ä
A³Ë?ÓÚ(4Òo¤?ºÈåWL?µRÝxµt?«1·Œ©AGN3FGL J1553.5+1256@7ɁOP @Fœ  0÷ðÀ8;‰‹.œËÀ;8±0?õÄ>£©½Ô@÷A\k»»@ÅÂnoI¿â]ÜT)¿ä")y1U¿ç+µª¾§h¿éÿì²£ßKAGNfsrq?ïêþ'д?`Ó¬‹sò?`pEéuÔ?_ø»˜×0?BFÍß'Ðê?:'xÂÖݹ?ïµÃV'¢?¼iB¥?pFëۈŒä?pºÆŽ:?t×iöI?zsß8Êé?îlWÛ? _Ûc¼³'?¥Ôí>t?šÙ…(.®z?"È¢âØu?‹‡ÿÑ!"?ïµ£³×f?';<Ðëï?[ÜNOO?`ÏÞr7:4?~IîýIzq?E_ʱº±?ïó%u¼ç?Q¡	¥F?U«½'+?Pýø%ó´?0%_%£V?'î·?ïᚤ(
X?gë!˜ùX?]ðcJí*?VEëe¡ìæ?_»Æä,D??`"À'ŒÅÊ?ï®4¹Ï?Žpì4Êý?'Ÿ¥ƒOÜ?‰€0¶b?ƒº	e¬D©?z
Ÿ»Z?ïîâÞÔY?b÷'3Q
¿?KTÐðܲ?K~š¬ÊCÒ?V;órSe?`IwßëÌAGN3FGL J1554.4+2010@@ÐÖ 2¥o@Gß<ã.À:E‰bÙÀ;Êô¯iåw¿ñSÀßIý@–Ehƒ@¢à?Ee¿æa‰iÃ	¢¿âԗ.Z[k¿×&;ìϿ簛µ
ú{AGNbll?ïç§ôG²i?bÞËpŒö?X$.°ù?]®Î³¤-?X‹é.Œ˜E?S˜ *V
?ïdÏKñßÆ?•ô÷4ëŸ??"	Ú+}"Ø?Ü +8zá?'ÂRÕúÅÇ?ˆvÏ«~'e?îtl$Ÿ?'š¸j¤•t?Ì
§`ì$?€uut4¨ÿ? Y`é‹?Ší.Î?îyÒÈ?—óZ›¦ÿ?vC$20t'?u¹‡k[Ó?¥§~WËxL?–kÔÙCz?ï÷Á²‰Í?K\±b_Yû?>»øqÛg?=ï>ýˆD4?D†ý蘱?E'¸%È^?ïÓkö%ê(?v³–'ÔTW?fpŠÁŒjC?leÙönmY?f#:光?i*v}¸ ?ï`Î-íE‹?{]d÷³Ð±?wÝ¿àÁ{?nÚõê0k?ˆ…¯
?rsLvMÖ¢?ï®]-ç‰?rZèvµ?SíW¾y>-?I`.Cnµ?êí»¯?q~çë¤çËAGN3FGL J1555.7+1111@5ë€uf@EúÕߛªÀ6‡ÜŽá¯³À9Øoàb«Ç?ëXlQ?–@DGw7ïÛ?øO÷øµ¿Ñ$¹»Öô¿ÚbR'¿Ñ§—U"þ¿ÑAЉ3´§AGNBLL?âFm6å?Ñó©Ã»ß?q:Ž@Ôí<?tXL¢O?Û/ì4,i?ÑýVõQ¤?ï–ØlLß??"¾ì›?uf¡V8[?z«NP+Ï?-±N¤ Y?ŠLªÇw?ã!Qù
Ý?·¹\#%U?­Ìt}Ïec?¡ûÖä7¶?ÕH.̊÷Y?µ¦k̅=è?áÆóìZ?Á͇È5ä>?z…†2¥Áà?{eÓQGܓ?ܹ6Ü¥?ÁàÒ-Åò?â"iýRYG?ÑÒ¡$IØ´?|ÝY<Š?'ä/¹K|?Úc¶ŸJä?ÑЗBÉ¡?ïÌ-'Ía6?ƒˆøÕpâ¥?f¹)µ»£,?qbEÍC/?mD¨Þ&ƒ?{ÁøgÃ#O?âEó^~\õ?¸ñ™/ÈaÜ?°MÊ1Ö«?¢Œóњþ?×`¦·"?·ÅýÅ{d?ä ØÔ±·a?ºօýW?ƒ¦U
©Xû?v>}eÉ?Ö!­t[¶?¹ä¯#ö)AGN3FGL J1557.4-7040@sÓIàâiÀ*QGàiaÃÀ9²ªÿ«1À;¦™_·öÀ	)^€"ä#@çÊ´èª@h(ÿӊV¿åx­Áä}¿â¿"nÑ3¿âÐ*æô¿æg¨MðŒAGNbcu?ï†ÕÒYÿ{?–ó8Õ@â?ns7˜
Kš?rrßUÆr?†­½y-úu?•}^ËH†?ïeä™9D?•kù=.?q]—62ò?|ä÷ÅØ?Ø3<«G?'÷s©î?íM<ÏN?¡v	î&Ÿã?™<ð*²Ì•?‰u.&ð3ù?®ºö²?òïM	°ô?ïcï"wJ?'Ý'Q©jó?$VàÁr?Eúªqí4?"Ya¶¢j®?'ÆÉ^ wÄ?e':Ø?µ¾´ª°Üñ?_ ^ÿo¯a?"˜³»dã?ŠžZÆ
•ú?´˜Þf[?ïËIË·4E?yBòq`»8?ZÝÏ%ÜüL?`Çuõx†/?s£¦s«Î?s•Éàœ(
?ï+CÛՆã?…U\™W+??'"kú¡ß ?rVæäI™é?'†N'&ÝÑ?ƒ#BO*Â?ïßoãMþÍ?p@ÎÙlÅ]>Ûʋƒó\Í>òbpX®W©?pAÑ\F"?p>Ä<)®ÕAGN3FGL J1558.9-6432@tøŸƒ¾fÀ!GŸÕó½À8ÉÄ<ÛR¢À;@cÞÌ©'À¿^\¶@fƒÂ—¿¥@0K`{•Î¿æ륙=dv¿Ö†§qüû¿á}PPB¿ÕÚiýc‡SAGNbll?ïÃÆQ;:?sh3_CÙ?\ž³þÛV?RèUÝù¹?wp±0K?qÝó´â?î›È|b(?«ÖçvÔð?}'ŠÏo"?"íœ,Y0?¢"&è?¨¬Œ‹J=¿?îkp*NL?—''¯ßE?˜ü|ýQ…÷?‹hë>…?¡û
'!ô@?ŽÒ'Õa?ïoB>؜©?ˆôÓ'å	J?ýå¿úÇ?&ˆWËÛd?'ºBÒ$µ?ˆì:ÊX¼?ïæüªÏ»®?^;{=zjB?O>\­0¢?DL	«µt?a3¾Rqv?W·9Ö¥?ïƒû¼?˜Ñ¾'ç¶?fw%óߪ?nû:Ý&"?‰ ý£õ·)?–::fíÅ¢?ïFH…™¡@?…1sõ®
?†'ÿÛô±8?~ú·¡¨?‡ÚÞ¯äŽÔ?vb†'=Ë6?ïÛ¦ý¸Û‡?gy°Áæ4>ß±¾:"ú…>æqûø!ˆÇ?r$"Ñ04?guìï>«#AGN3FGL J1558.9+5625@UäÉ$.@FàxÀ>-À9DËüÃ4žÀ;´Sø¥˜«¿ñmš}[F@éÊ@®êÖù¿çè(Z½ë¿Þ–÷Üá¿á·_öW,¿æŠt¼P¹èAGNbll?ïùËÓÁ?sÿ	׍y´?'´ºãò/?ØöhtàQ?E`]ÅgÊû?sû^ÊT'A?ï¯ýÑ¨?‹/¼TR¾?s£{¨i~?"©ÄN??t]›ÒÞþ‹?{žJ"»Ã?ï6:¢páG?Šç´'¸7?è;ø݁?wŒœ)š™Ñ?D¯ÀY?†">"Bö'?ïµ½co³d?{Á@~‡‡?HvÓ¤Šìá?RF{¨ÚŒ£?	9Ù ]e?{(THV±?ïê5]¯Þ?¥"âiRe?R©€SŒ	?04ÍNF ¶?e
Eæ!³?¥m]}>?ïå2"ó^Ô?f8p:ÎÓ¥?WŽ•ZøЈ?TM²µ$\§?^BMG?_bL¯?ï¤XïãÜ?}eÔPêË0?qsÀ
:L?fÞ|û8Òþ?|€Ä¸5£ì?z¸yç?ïò­}bg?]>7åFÛ¥?®'v9?,E&Ùc"?XÄÚÓ´<D?\çûõßAGN3FGL J1559.7+8512@]·Êÿm3	@>TDŸlArÀ9ŒO"}ŠÀ;䰔‡áá¿ða5Tu£@{=gµj@ϊ¿Œƒ¿æØß/®vÿ¿åõ³ö3šÚ¿ß´2¿o¶¿é~ªùF&AGNbcu?ïÖÙñÖû?p¯7°"c?jeè‹õå?jz­§©¹?]€K<Ýâ?YšµÅi—?ïŽë"Šù?‰¸ËV|‹?wáª^s·â?r("Å
!?€TFëGè?…bz|%ý?îö(7£ý˜?ŒúqfC?Šç·V:k®?€tÄbÌ?"ÇcÒ³"?ƒ'W8ñ0?ïo"di.?‰6óºªé×?aZÚv²?duÁi ?ÈuíE|Ý?‡Þ<HÌÍ?ïó‹{¸w?QdXWw'?Rè)Íî[?L–…š‹•v??<áÿÞ(?9P•±®n?ïÕÐdJÇ?q °ÉèØ?cD•G°±Ï?[dP¡ôØ?gškaÞþ?k@\¥×?ÞEŠ?xQ<ó£ô?x/P'?or8wWà?|€n"¾?r¾~kÆ?ï胿	7.?aõ2`i;?6H
‡$?5?Ʀ)J?d³@9¤?af·Ò¼rAGN3FGL J1559.8-2525@u¾q'l@4'	€²BÀ:lÚÌiÐ~À;ž
ø†¿ã
U€1‹
@€wö[¼i?ÿ-€kË*¿éäåŸxù¿å^â8³•¿ãK±së?­-ZoüÖïAGNbcu?ïíOLˆ3?[X)EIdf?6ˆSïw?1ÉüRu?`­¡v¥S?ZLŠP"?‡eÔ4?‰Æ²ê>ï?rXÖíúO?vc"
›w[?|%ãX›GÓ?'í/Q¤¨?îÞo^:Q?…½\›qß?‡Á2B?tcUôx¤?˜µq"×bß?Yø#£K?îé߁§¬Ï?•ìÚ{:ž?FÛ#‡÷?OëM;v^³?¡	"CVÉ?•âdÚ7S?ïø»Æ6¨?NŽ+Hfè-?)"#xšÕ?%IY»­jÕ?IH	ˆîKí?Lt1¢u2è?ïÛ¹ªL›?r"_cm?_)­Çz²·?bÄ?d±'t+€?gÃhöe?ïw™۟?v,þ¿*x?y-¦ß+å?a'-Kªá?…¸ßZ"s?rz¬}þ±Â?ïÎÑ»¸Â?lNJuúð?,
³ËœL>?-‹ëåÑ´?w¶´cr¶Ä?l
敜D$AGN3FGL J1559.9+2319@CTÇÀ'á@G¸b`GhtÀ9玦 ™À;›Î­wœð¿â"'p³v@µ
eÄ*@ÍÏڀÀ?íÂÀÜÿtë¿á-v"q¿äPcxSŒ¿Õðï
(;ÍAGNbll?ïôtjÊ_?NQ`ó)þG?DÆã-u$?D£¼n¡?Ii"ת´?@ÞÅuWß/?燐ÁZ9?Š<Y	¢_?s@~Ÿ"º?'¤êŃâ?xè ¸Ñe?€—þÐ?ï½»?‹ZÜò@??Š'Ë‹†?"µ¿;'?'‡>·?€OSu
#?îߍ¶®Ê¦?™8®SWCr?cñáã!?a=UÑ»Åy? ÖåyrÛà?˜ô̕üHi?ïûÒ @¦?5ªjÊW½?.+
Ž…1?&=•Wq±?2Yw™Ð?,¬®x­?ïã¹÷:½?iåã˜B
ú?Y›x±_Œ?Tù–ôÁ?`/‰´5—?dˆóEêÀ?ïˆmhÒì?zÞJ^Ú??~uÄ@vé?u¤iPƒ—?}S‡R£r­?ei±cS¦?ïÎ1mO'Ÿ?q
h'™¦?<l²#àã?2?"ò>A?w ‡»ÉåÕ?péøèmÁìAGN3FGL J1600.3-5810@t\3¿µÀu'1>À9ìæ˜Oí~À;KRü&V¬?áE'ÏiÕ@	d^¤P,@Ô?\â.¿âÌ Ë¸¶Ñ¿"îj+lë;¿æ}†Ev¿àpLžÀ—AGNbcu?èœ0¨œõL?Ëݖ˫\?yŋ! %‡?'®ùëz?ÌÁ&y€?Ì&ð"À*—?ÎQãúˆ>J?ÐlfÃáõ1?Î(t¤}ß?Òôu—?àê|ä4Ðö?ÌPe›Óä?ìcЦ÷?£Üþ›—nÉ?¥¿+ÐB—?"XZÒ±?´Q`¢D?žw¦'–ê?ØÜ»¦Îz;?¿'cëóê¯?Óÿ8œvH?Ãûj¶?Ó$¼»v}?½ÐB(Ðü?ë':øyxè?ÇØÈxÕ(ç?cf]'/"©?p]xЦ?Áiz¦þö¯?Çí³˜Gà?ÞÑ"yt§?՜ˆ®²&ü?Á´íÀðÔ?¾\¥v¶Yˆ?ØTfþ«…ï?ÑO,Ÿ+
?î•9øõÐ?'½£ uM?""ÎY'W?"'
Ôµì?™Ô?'øž?ˆ?EÍ(?å
2i<b:?±â€ÑN?ƂÜ5Aø•?®D1+rÔÇ?ÅTZ#¦½?¨}øš¯9MIXED3FGL J1600.8-3053@uzÿ°Nè@0uS€°"ˆÀ9Цã.8À;É,.\4?÷>¸ŸÄ+@PRþª•?òšª8"[J?ïþ+«™:=¿Î²¢¹ÑB¿ÞTn#°¿ìbÇÒßWáPSRPSR?ÂýL
k?»á'2í	¦?çÄÛr,?Ƈ»nO?»å␌h?»|†"ïCD?º±LNô@?»7Ûµ.0Ñ?çGYñ>?ÅÆ#£¦ÁS?Ť
õÐÀç?‹y£k;?ÐëL%Õ?¸0g3½]?ãçk	ÊjX?ºiõWS?ÀJ}>fx?©ð?ÂêK?Ï2Ñ'i?N?´4ˆ""®?ã"î
±Ô?»Eiܛ*?Âyv¡Ð}d?°•
 #?ÏnUÕìÓu?žQȘ¬?äcÚ['ÝI?Ë8Æ­µ?¾sKëÖ?»^GúF?ÍtŒéKÍM?Ãw§Êx£?ä1ÅöL€•?ÆJÏý-èœ?ÁÄ[='0`?½à¥"!ç?Úº¢ÿ°
0?µ8¯,ªE?ßô™‰S?µ¿Êæm²¶?¸õ£™mfð?£îïIiú?ÚNdºûÐ?²ßâˉ"J?àˆ¿-õ(-?³I$ù4?²'þF¶V? ½Š8Î^ºPSR3FGL J1603.7+1106@7ôàM/@EfÀ(yœÀ9ÑøQÆÀ;{Þ-G`è¿©­‰ô1«ú@,f…›
@˜¿aÕ2¿Ïû/i¿æÊ-ªL0¿ãÕÙE"–O¿âïHïíAGNbll?ïúelžíI?:æáÛIŒ?1›"\m]W?/s³€m?;9_pÙ?2ÞéÑP?ï¨å(°š´?Š/¦"ù[?sÄñ3 û6?'Ô(3lhZ?wÈzccž«?}¢}éo-?ï@}RTûI?ƒž#G-•?"Ôâˆw²?wç
º+¡ ?‹Èð{&?{]Óðgî?îãû@ŽÍ?TÃ`C_ò?iB]mÒj?b,ÍÂÛÒ7? :ªußÖ?Œ!XäIu}?ïõ#8qê?œŽ¸âV™?+3ˆ˜?6F¾Š,"™?RSùVê?šUie?ïए¹=p?g56bþ€?[y!@¸?SŒ9s@?ažßëî¿&?bH'"ò*Ÿ?ÐËg¦?|Ov²ÿ98?ycô)•?u¥Ž	]0?xD†¯"?l¢Å?\µ?ïÁHd°?iÑ¿Wpø?SñÌ8
ß?@[ècn2?zhÅn82?hjʶ^¯AGN3FGL J1603.9-4903@t™€o&)@Œn¿{UŒÀ6üUFƒrÀ:Vól|*?ÖØÛ~@w¿@ˆY«B@«ÿøž7¿ã\̀—¿ä©a÷}
Ô¿àš¹yÞ¾<¿Û+I¡AGNbll?íñÂH#'?±®>bky?dQ0x£ú?cn?½­?¯žÈtÑ͸?±vpªÐF?麈¾Ö?Ðô¹ëžŸ?'«žF*?˜"ëÜ?X?ɛ¢^Ô?Ͻº ¥Q‰?ä€úÃÍl&?·@¦z‡îg?£â÷Æ?–‹­Mo?Ԏ&{aA±?¶FNCßò§?ìêtÁ%­A?¤Ë®nÓS?Pf|äÄ?RV¨3Šxï?¸jÁÔ߃?¤ÅË ±B±?ïžÖD?"#Áöæîå?a¶—'¶$?k½ï˜3}?ƒÜöOüçM?'·T`A˜®?îM¨RL±'?º+¬IR7
?|{,Ic?ˆ¬j2¢	m?§–ÙáJm?·'cq‹ÕÙ?è\†Zš?´Š]U_qÄ?£MSpŃæ?—d^óW/z?ɼ¤­ì.^?²Pê¬gF?îÑ@žøön?‹ýIS˜›?Fø¾e>?@f øMy?¢$sœ?ŒŒˆ%AGN3FGL J1604.4-4442@tòߋr@|€.8£À7µ"k4+À:ÃÝo²?ƒ?çðû"'\@7£9€A@Ÿ­@j~N¿ãª]ÒÝÍ¿çå)MèQt¿ã–È6¿êÔí¢QÆiAGNbcu?ï†Tèå‡.?ŒéµÎŸ?rcs:©Ü?u›Táù?…9Cúrûµ?†‹ÖIRx?îa'ke
?¬ÆÅ&X?}IrÍ@|Õ?}Á´à°Ñ?¦DZíŸEÏ?ªs°9œT?é`ù4èG°?±1å'º?²¢
''M×?¢–ÁÏ¢þ?Á+ã:T?ª1Ŝm8²?îâ—S2? 525)Ø?q±»üQi?s=ø44à?­‹Ÿ
ªk,?Ÿ"üŸúæù?ïÑ×Ç??"Ðèõ©8>?aæÎ×B4l?u~ÖhCl?lB&Iτž?uÔHsa£•?ï\Õ¼-‡?›'Óµr‰?nU4ïÌO?oÞíH[Ñ?š¶.¢?˜'~U7ÃO?ìrvŒú#ó?§MÃj?¨m€f5̽?œ>ô`ö?°5‹eú
?Ÿ˜æùñ3?ïaËT°9!?'9e1)š?cm¿A|?V© …"¼?'X݀'ü5?vÛRCh8AGN3FGL J1604.6+5714@V(Àª'@F]K 'ßÀ8¦'w"ŒÀ;'ìÝ
?õ"AöðaÒ@•‡û6——@žð86Ó&¿ßŽ8	¿ç?Î)̵®¿åò.XŸ¡¿ë{ùJ¯&AGNfsrq?ïàŽD?¹Ã?fJŸ;¿%Ê?hg¯ð}Àó?cwÚ¬ZMÁ?L(.¥3p?L5ÔçlúÌ?ïÍ_ï©Ç?ŠPWðҜ?~‹‡P| ?{Qã­J?€ÆädÖA?ƒsÙ'#'?í¹ðá:?ÓÙÃL,?§Iqf‰G?—Ò´ÏG?™Ä︴??éxÕ?îÜc»ÊÇ?š"¦5´u?*ý>5™
?‰ØÍ<µý?"Þ
£¨˜?–(Éœø;?ïíë"?Y¢;6ÌÃ?`1û,¶W?X4CÌÜÊ?5°Ë#,I?0x®n?ïȇ¥BU?v!‰&¬ª?lxìçӛ?dnƒ‡†·?jÿ''&ŸL?p""Ñx£?îËÅí¤L•?'"§Uâ
:?š?1™*3?ŒRK°5E?ˆâDè'P?<𯫭Ü?ï¯à©‰·à?x-,<­³?yµ8~õ?j¯VQÀÆë?l´åšº.?q'ßÖ4@AGN3FGL J1606.1+5630@U̚ÑVŸ@Fdä`gHäÀ:~À?öÀ;ë¼Õ±À $rÑç@Þè<k?ÿ'N^²½Ø¿ã«;þ'sŽ¿èbÅ'øþ•¿ÜÄò]€
׿ǯLý£sAGNbll?ïÛ"㯽G?r}]C=¤?2{Ò7m?0"0QbmB?qFÑ[?rL9EoA?ïÄ7 
ø¢?|œÐ<7M¨?j>½Š¤†?mù!Ôºüœ?pÔРm¨?t7ï"O¾;?îÛގ§^d?‡ŒäǘÅ?ƒUÿý®?o
£Ò¶Ò?šÙ.›N ?"!	@?¾?ïÝt¸
Íô?m•"B>ëwP««uR>õ~Veó0?q7èXªJF?m¹ôW©(?ïö)3nÜ?S€ˆ¶Pi9?"	Ù Z?D–xqQ?Qlu`â"h?R•«5ð¡?ïç4RÔŒ?e·Õ=
Ì?Vˆ0«Ž?T›­+
´?[)€¼Yá?_ýtæá"?ï{•]Rt?rῪÿ¸Q?v¾	F?÷\?_Ôx™˜¿?…»£û4x´?n*©úi?ïú'3ãv ?AptÍWò>Ç`JޔÊ>>Ê@²rê?EŸÐ9ôÆ?Aj›¤À¥AGN3FGL J1607.0+1551@=`A€ÓÏö@Eµëž*ùÀ8kğס<À;]_Âví?꘴îDýÇ@çL‡`\@F¤‹¿á—:2›¿äE0X.ã¿äñšÃ‡¡¿æB7Š°ÈŠAGNfsrq?ï«<߄_v?…qIæ U?€ é·A´Ñ?ƒðë/Ñcf?b?yx@?\"}¤*Í?ìÒXƒ`…?º–Š'T?°׃¶¹?³|Y´$ªò?¢¢jøj:?¬äÓnpƒÈ?î}%8YôÏ?—­[ÞÇ!ò?—àÍôI?wô
b?˜½xçŠwÅ?`ªULºM?æ	€K·/ú?¶ªËK©‡ß?Å°"L€a9?±-`Š7÷?Â)z"¢Þß?±B©Íã0?ïà¿Np6°?pU{I»?h)2dêWþ?mÝwè`{g?L]û¤&žV?GÀ
G?îâcÍYåz?¤Î—¾}G·?•ÎÕ]–.? ÙR<ôä)?‹Éaòß:?"óë.=©O?ïr5˜yo>?"µº¼ãR?'!ÎR§ z?~·¯ÄÊ?Pˁ––!?w"ŽŒ«£?ì¼æ_ðÖl?›¼3&¼åö?¯‡\î'n?_kC>?¤ª=[æÑ?"ðþ«I+AGN3FGL J1607.9-2040@v, <K
@6""?À9½¼{À;bYG™ò…¿'0ÖÔcø)@
c-ÜÝ<@?©c;¿Í2=¨4ō¿àæNè订¿ØØ©òçz¿ã²öЉùFAGNbcu?ï¢&÷CK?'©E`a?h7¥m̅?eײdæl?h¼2Á¸?jÛZJ?ï:WY®3? u0+1€,?ƒòf "*®?
äΐb?wÂü‹Î¢?œ#µP*u?î#ƒ§ƒ¬?•N+âÌ?•gö…_¦?"_½fe­3?£ìÄ´±j?º^29?ë¶ÏZ¤Cõ? 
p׏°?~‡µåY?'!¨­Æê»?¾Y´3EI-?žoŽÞH­ë?ïäë}'ü?dH(8/}»?M4
ˆº/?KÇÈ0=Hp?d}ÇOŽm?`Òà–dý?ï¯/"±í?‰Èz•êf?pɑ·Øˆë?oß]úƒS?wž£×#ª?"Ë^óp¨?ïHLû¹ÒÓ?ƒ+ݛª€?"}3œ	—v?w2bQӍ(?‰ou³à?vï!ã¸ø3?î¢ðЍ º?'g ÉÛ«?¬$Å?fÅ3K"ýu?¡eéÐÔôX?+ËiAGN3FGL J1608.6+1029@7ÿ·ä@Dh _ñØÀ8‡ôafLeÀ;\¤£¸×M?ôXO´HG@_óWûêr@óÑ@yí­¿æˆ{QZÁ¿æû…å\»˜¿ë	Jƒu¿í¯|¯AGNfsrq?ïÔéa#q?v1˜kÎ?rõaø·Ç
?uÓT1Õ?D¯m50¿?Kº©æçK?ï:¦îRÚ?–g")ô¼?‰Ïo±—%ò?‡4ê
<Ž?‡†ÔËïh?'à0Ç?îA+—lÌ?—Âädű¸?£ñ9Ý?"¹ {(H?' ½¤ÆÄ?†
þÚ½°?í7#@)™_?¦¶ŸuÒ?¨¡!¶ÿž? Óÿe>ÿ?£ìªH™÷? C›˜Ýi?ïÙûw7Í?q©ÖPú±?qz¯¶øãI?p¶%Âb‹?8yKÜÂw?<k× +ƒ?ï¬TVïP?~:mÞې0?u5µ;+÷?m†ƒ&ºx½?t J–!Ð?wך`\ïÂ?îþûÉ?'us
òY?ì¼"Òà/?Œ¬#X ‡È?‰ú›M_?|h-0Ìé?ï;S׏ì?ˆÓ¹Æ¢Ë£?HM Ó?}Þ
ÆÚÔ?Zb]S~?€å;dú:wAGN3FGL J1610.6-3956@u3¸Ÿƒ¾f@ þ{ßõH—À9ä@†ØÍÀ;
þ®Ç(?Û>ëÙÛ@(¬~¨@áé€aº/¿çþöjªï¿ét¢ #¿æZ||¨¿ë§"÷ 2zAGNfsrq?ìÃ0öÂê?¶!¹õC?«‡©Ùؤ?ªo'€'åà?¨HpD&C¸?®OÏE(ýE?è`Å}«¯ú?Ê¥ßÀWÉ?²XN$?±kTŸ°?Åw=úŸF?Å…Î5­Œ?å®ûÅL"?·9Á¾b ?Á#ñ®¥ç¨?¨^T'"º?È :g?²+†cÙY¨?â:8R¬Ë%?±î¨°?»»¾1©pQ?¢YÕ@©Ž?ԜŸÍ),ä?±B˜‰4ƒ?îÎO;Û?¡ˆ#™Ì?—}¥2¯È?—…í°Á*7?pæ£á¼¶?"0À}Ž??í^(R78?¸'fQF-\?žJ•Í?¤{)Wll?«òÜCå?°pŽEna?êøá¤d?ª¾õif/'?´x…š*°? <žœÜÆÊ?´0(nú'¿?¡º|8ã?阻ôÉ|G?¡†vp,Šc?±N87Î?'»ü1~{?Á…†ù??žps¯g6AGN3FGL J1610.8-6649@t™÷LÀ&J§€âéoÀ8[#'Õ€À:ìHŒ`Ì?êm¹'~[6@¤­ùwû?ü^¶­yö¿ÜxŸ
Î2¿ÔwFÀP4¿Ú»¼œpR¿Ñ3þÜáº<AGNbll?î/\¢˜F?­Üæ
ëÛ?ƒ5zw¡?"#"åŸ?¨HWeJ:>?«L`Ö¯y«?í«*ÈwõÒ?¹ƒBj̓?JÕ«˜9?'ñÓDŠ?­úž
O`Ò?¶\7ó§Ñ?í-O»Öõ?£ä¤:™O?—çCìJä?ŠÃV™y?/?°›²X Ý? ã"KW?ê¤S?©vŽZSç?Œ–C
Ý"?ŠÞVTMô¥?ÅåÚì¢?¨Ï蹃Å?îËOƒÃ:õ?¯Ûã `Λ?~P|ḵé?‹Yîÿÿ<?Ÿðn]Bá?ªêM¼üi*?ï<àRˆ?¢v‡ñ¦uö?~ñ~›†Â?‡BÌ>˜¨>?•ÜUØ­3?œH²o€Þ?ïâHŠ?Œ9}{á	á?†YùèÜh?€7ëž»?'/Ä8€Y?"hBÀä&?í¯ë,UÀÉ?'[ãÍŸ?†ÔN‡íß?u
8ë·$?¯L9·®Bù?'IbÇ
ñAGN3FGL J1612.4-3100@u¥ 8L@-JÄ!, rÀ9ÌÎFImÀ;—A¥Ãt?öCÞâ# A@"1jÜí?èÆ£É&Ð?ïýϘÑj
¿·l'ðû!Á¿ãÊ"Cñò¿åàÜ+íøAGNbcu?ëìÕÜ9?¼€dÙe?±"öqê\?³ðuYÀ³?®"QÊç´?³,,mÚ«?é÷¡PŒ?Ë裆Ç?¸·¾d•†?¾çuš‹Ý?¾¿YÝ?ÂÇû?ä;'᥈?¶ÜÄ/éS?оʑÅK	?´hú±GÇP?»,É)ݧ™?©ê®ç·ôH?å-[ÙÖ±¹?ÀMR¹©?ÊÜ®Tš>¹?»'Žå5¤?ÀmâAå8æ?µ©pò<?íË…âë?¶A¾u_í??¤ïá»ü'ã?°«zâ\F¡?œ¿‹Ò£ÔÆ?¥ŽÎK†?ìÂÓ΍…ÿ?ÁÔI–ª"?ªŽ¢}jzL?´ÙƄ!@?©D ˜á>È?´'lÑøK?å¦ÞÄ"p?µ¯8Öúç×?ÎËbê8¡?³j^è¨Õ?µ2
I9?¥®&Ø&µ0?꾾෠¤?¯âœékz3?¿oÀñæüh?¨ Â6S §?¥4
P`ñ? 7ljÅOÑAGN3FGL J1613.8+3410@KŽÀA¤@G,|?ìÀ9…'Uþ9VÀ;ۛárv?¿¯½_ïð7@.ƒíŠÝi@Кßê¶Ã¿è$¤ˆœ,'¿áÂÓþüR¿æÎPZ‹¿ÜÌñõ-xAGNfsrq?ïÛô—Žsî?lk.(ˆ?hú¥äZÒ?fàC÷½ó?WòÜA­©?W3Š–#qå?ïtÑx®¡?'`b
àŒ?›픍'?ƒ`¼lN%?'þkÇ·*?Œ2âºÑ è?îŠû²[ ?'aÑMO?"6ï¦!¯?†\ÔqzÏQ?ši¯¾k'|?‡1Ùßv'?îŽI׏s{?™¸Ú&§‰œ?É)Xc?Š<ÓÚ¹ô?Ÿuà€(œf?"áÛ©¤?ïëONUÀ?"<Ï>A.?N(/
¦?T]…že]?Z`Ð<%o°?"káùO?ï҄^kg¤?u趃Nou?dµ…o܀?hryõ-vØ?hƉ‡ø?n{åyx?ïi:V=#w?€|ù×C1§?ƒ)ÏÀ?xÆï¤Nd£?'¡Mf"ôp?p·[k̄æ?ïÀbþýÌt?r2©©à ?eõ2²KŠ?UU•¸Ø[ô?tÓçzÐd2?oQèè"ÉóAGN3FGL J1614.5-2231@v	ÄupÅ@42«@‹
‹À8z½ø³oÀ;;…Ÿç't@Bv½K¥p@&©fÁ*,?ò˜(Ë{>?™È—«OF¿ÅPVHzÜÚ¿å³ìí\[Ü°×PSRPSR?wÎÖ½;ŠE?­ÙûO?ï"GÄKF?'7É¡{?~GÂòŠ?Š|Ë«Û'¾?€#±O3À?Žµ5—Áœ%?íüœx­¤?·³aª
?¬-L(ŠÂ?¶uÊ5Ü?ºÉԚ­ˆ?"2áp÷"²?ì0n‰d\?©ƒ£üވB?·
ÙAnB$?¦@]× ¹?•ðËË:û?ˆ²1$H?î×Îh?¡,²
úV­?¤Ê)©M"ÿ?›VLkòÎ?h¨l…ŽC«?týãCÔdŸ?ï"üÛ¦%?œD<¹Òq?"Ö®%i®?™Ñ—¨Kå¼?Ž-çhW@?˜¸
ƒ(b?í–.Ê»?µû-or?¯™yq¶?´•ŒÁ/e?¢šåWs?—­ˆœ˜¾?ëæ`,n%«?©°[ÉHæ?·ŒƦî?¥ìÁÝ %;?¦†Ös¢a?ƒ=}21‹?í¤ÍÂôg?šøRcY~'?žZñ2`?'âa¦¼vPSR3FGL J1615.3-5146e@tº£3v¿å‰€5´1À6ï¸GʐÀ9»–~\&r?ï$&O­@þ°³¼…'?ýÔ]àZô?ïýßÉÿ'ó?"¬'ßZö¿à'7'߿ހ¡{j×OTHERspp?³`Â-¼š³?±¹Ya?¡Ÿ\À	?£œ½@‹ã?ìyõĊ*ˆ?¸eXÄC9±?ª0¡â­"§?º4!£Ft6?ÀVÎES–?¿Z£z?êGBPK`À?Ãìi4ÌæM?¾Q‡'ô?©Š‹Ø½{3?¶Ùؗ©?¦'•#Æ·?éaÚÉmOl?°ÒKÿÂId?¿rFGÑ¿•?´®¨¡(Â?º¦Q_KÉ?´±?,l˜Ð?è¼õLÙޔ?¾w«wI?»à%¯'þp?·ÍAϞ²? ‡f*|Ï?žØ°3M°?ë{"é'Ý?»¯-5B?¸Þÿnÿtç?Á×%UÏë:?ÆP"¨W?ÀQÌ8ÛÇD?çP1x?Çúà¦Œ?Ã'ü úâ?°ÖâÚ2?¼7Xíé
[?¥Þ váìk?ç¯N㟜?³&œXp"?ÂèÚαî?¶Qd+æ4?±K!«:D¹?¢Ç£Œzç?éeì;ä?º.v"ÅOTHER3FGL J1615.8+4712@RwïÝëÙ@FË/¿á+ÿÀ:X¤ï81 À;ìGJAl²¿Ë•ÌŸDB>@@q@)ªo÷µ?ïÙÖɔ£¿áòT"¿ÜÚòaSN~¿å=†uûYÓAGNfsrq?ï÷¯°BŽ¬?Hh>ð»q?;z3þæ?4É
v"NE?C¿‹U½?Avڑo»ª?ï}\Z°?_Ù²Íî?€_¦ÛUä?…ºØ…G$?€IBm¨™ü?"…ÕWåä?ïUÇ> *?€4U›]¬?¼/g+?rèöÙM?ˆãÞºŸžw?uì7ÇHÕ?Yj:Ã?œ"ÚLnþ?' ÁS]?x¹Íl^é?¡œ·$QÀ}?š/wŒµwÊ?ïýQ~Å$Y?-Xü:)?!ycèÀL®?çcùŒ?)n°érvÔ?#è{̑ó\?ïÔÊÑ0Dý?n¯ìüžõÅ?c®û$&ç}?\;T؈?g†3tš[^?h0'd?!C,â?t"§Æjí?vLK;?ißÑßͯÈ?{"p@\/?m¨ÜŸ×

?ï½U©ˆW°?sü
ŽÕ6¦?c:¡"K?S2ú'#¡Ï?w·ÚÌ8®?rb<ƶ¤AGN3FGL J1616.2-5054e@tÅـo&)¿ÀÈßK³À6"`4óþÀ9ákÀB{?·ä»uÊM@ÖSI3¦@(ˆ!ö¿áí¢F¼¿æ‰u_'®¿ãg–²^Œ}¿ÝÄ&¤`OTHERPWN?µY$µ´/Ý?´#4Ù+ç?]¯ÐH‹ž?geŽáïó'?íF-«Ï?´kÂ7³Ð›?Ξæ°ùˆ?ÒJç"ú"›?§q™wð-x?¨GÿžáK?æá_îýú?Ò£‡%›?ØÇ
6uï?´qjk¸H?¦þàWYˆP?šuzoK¬?â,Œß].k?´Ú‡i|?ßÎæ{[?Å*'¥º˜?[ªÕqÓ?_®Ídgv?àiCUj?º?Å+‡Yó]Ó?Ϛµ´"8?Ê3D½–›Z?rOÞl3é<?whg¤ROñ?çô²ÖÖ'?ʁÁTÀï?Ö1ÑÎ?ÕV"T´{?¬¼ðxÝé(?¤TÄœê?â¼Ý4½»§?Ô	áM1?Ùþ7gd,?µMŠjó+?®QAS@ö"?žáÚ
¹²?áÐ6þ]­?µ%5Ç÷ Â?áÍ1+àÈ?Á,&A»¿½?]O<mÙt?S£]µaO?ÜH¨ÙV?Á.!×ÒJ¡MIXED3FGL J1616.4+4631@R7Ã_Ñ ï@FÈûÿÀ? À:=aŠQþÀ;סS¢>"?Ù©¹‹Á-¡@­N€@­@»0à¿éaˆcÄÔ¿ê«ËŽå¿ä֌]é6²¿ïÿس"smAGNfsrq?ïö£ÓYXâ?O %b	œ(?4ÃMk?9³åëØ?Kbi°?Hõçê,A?î¿uM_ˆ? 7¤3µëÞ?–TÍ®Ý?'uŠ+ù"<?'½9E–Ä?–1hj¾?îì¼b,¬?-˜CÍ?³"&÷?ƒ±_Púñ²?'´ä)³ù.?…tÀš…?ìô³Ž7eÈ?¢(8ùÞ¸9?ª<Õ¬â?˜í4fÞ<?¦x¯IqG?—2»	3Ž?ïû¸Þ‹ï–?<Ô*ç¢f?)#\Ua?+Û*nJ?5§IòM}Õ?2óÎõGÿI?ï£<àÛød?}wtËïÛ,?y­øR4öÅ?pD2qK°?t³—:ÿcX?tóà)¦bš?ïR¶ziÂU?ÍdtŽ:G?‰€5°Á?ydþ¯å_½?'6á.~і?võ¾P7ÆÛ?ï4
úú?€!7ÑA?ÿº4ï â?s ..ÿA?‰8µª?vÇÞ6½½AGN3FGL J1616.8+4111@PP9ßõž}@F÷¹¿©Î›À:"~êÁªZÀ<o%QÉ ?Ùf¯"ù>@Ù§b/'@ ™`
Ü·¿ã—"%ĵ§¿âP'gñ׿移*'¾¿ïÿWZýAGNbll?ë1nëx½?ÌÑzü z	?ÃJ¯'_?Ì×JzÞ©ª?o"Ï\Ló«?t-䌐?ëª"í…?¹AM;w?¸Ï®%-;A?³ žë&?¦dyâü9?©HÊ`?ë†ö©6'?¦'-[ ð¸?¸SXÒ:?¡¢þ\ ?¦éãȌ­??'ŸÐ3leš?蔥³s5?´²ÐS=_?ǹ/¥N?²øîù#k5?§ªË6ì}?šJ»€˜C?ë¢B¬Ý?Óe
%ÉT?Á3Ù´šY'?ÓnkøÕ?`ŠQ"6¼?b©[à¦Ëh?îÿ:ïPkŽ?—kΠ°á?""$[aÍ?'ß"½¼?‡(ûx';?‡FnUFy#?íÝ\Ãêô?—9Šc'a÷?¨7™JC?"ϬSš+Ç?"å4î6cp?}ÈaK~?îMœz
|?'o3›a;?¦5ïà8?Œ=n	BÕÛ?",	³/a?{Åî Œ5AGN3FGL J1616.8-2300@v	é€,
J@3w›ßÄ÷À9¼6YX`êÀ;73Ëßg?ìN¼9'Ùó@:zÅnÇ@Ûÿo·H?ïŠ3•XÂ9¿çŠ"ƒÉy¿Å7&‡ÔQ¿ïÿæPlOTHERglc?íÀþ¦Ó?¶ÝQ ÎŊ?¡DBG÷[?¦ÈhoB<—?¦¿ç'i?³e¦â}DA?ä^ù5ò'?Ðo"¶«£1?ÒÙßF™cá?Í°
""?±£"XÏp?µ[}Ý®û?åœ^þÃY?´<})Ž~9?ÌQtÁè/?²f?
×»?ºz%µòÛ?¤a'Hf˜ˆ?àoÖÖÕ©?Ãàºö
³¸?ÊuFh_?ÃÃè€:*§?Ò—¯MyÊ?Á~£kvèâ?îœòE?¶Nl}4g?•´\Žª?š'6ˆY?£¢l2S?³ÅöëtÒ?åá'IC?ñ?Ñ£"íëÞé?Ñ՝?Ða†z$€µ?©À.ƒËüî?­¹@\tFº?èãû?Úi ?­­–õ§ì?Ãüœš·Q?¨Ã¹,™×?°æíÜe;Ü?Ÿ9.÷<?åÅÈPˆ¥ù?·}%+Éâ?ʦs§l–?¶» uC?¼"Ö1-'3?©¶c
Þ¢°AGN3FGL J1617.3-2519@uî{¿"ÿ&@1Î9ßõž}À9(>Œ,ɍÀ;ç½f?ïÜÙ¤ƒ@
Þô¾@¹³ ©BÚ¿ã¥æÞ4Âï¿ê³'ɮƿåOI¥v®¿ïß²Ej æAGNbcu?âõ"Á‰Ì?È
+²¶K+?¼È¹âo¡?³=y7ÛUÕ?Òâ¨8:P€?È|k¾óxç?Ø۟F	'=?Å°¨kê?Ý^&ØB2?Ãd¾¡:ù?ÌsÃh—f?ÀJ's	¸?á»ÿ/p?·dOû
˜?ÉC[¹(?­F"ÜŽ¯Ý?Ñ4Ú&@uU?·"'¥îâW?ΆÎ
ÈC?°ÍnœæŒ?ÛR…0ßy€?¸Î¿¹Î0?ÕjÈ<wÞ?³S U¿\ô?䋝雡?ǽê,•Eˆ?ê@—&?¹¶8$£g=?Ì¿'GŒW?ƪ>ƒ.Ú?ã8I½/Ã4?Ãù «~?ÓL@ª
?ÀMf5ûØ?¹¯o¿Œ?¶ðç÷/'ß?æ°W½šït?±súÁBN0?ÂyŽ-Í4?¤0æn1ׁ?ÂÅÛÇ2ü?ªk'Šz¦?ÚB͍šm?¬ša%2Í?Ùb간å?¯1÷ýZ¼Ã?ȶA–Ù?£8 
•
MIXED3FGL J1617.4-5846@tp/hیÀ'ò€¯ËÀ8pº¼ÿÐ/À;I]A#·?Þª¶þÀv@n'!€-b@Þæ …Üx¿å÷ŽÔ'É¿èb¤‰ýè¿æ¶òI¿ï"äå-§êAGNfsrq?ïÍóØ¡¹›?v¦{~¢Yž?d+ÿ•}|l?géõrJ…?mà'Æ	8Š?qž2dê?è<¬n»ýû?Ë]JÀºè?©ÌV¥?¨Ðo©è
ž?Èś='8«?ÇO5ùK'?ì·‰€5´?¡Ë˵""®?§Òܑ}ûµ?"˜†Šx]m?¬¼šÙîE?š<a¼$âL?ìÇYÆDó?©a³_WB?šÿP€ì'ž?"RQôxê?¹ñ܎|?§­Èè'¯?ïâøanÚ?cAÞ}æà?`ç|éo È?Wý»ÎVj?X@D]»é™?Y/"@Û¬'?ìçLpØ'?¹Õ'ù¾ÿ?™Òd	–Œ?šÖÐ~)ž?²QwG£ò?³†	?=v?îEãóô»?–]׌ôc¢?œ¼òu2D?ŠUNk;ðï?š‡‹‡za?yÆhÐ;&?îȅ‡`St?'d¤ìÊHW?…YPöŠî?ƒGêî''Ï?œB¦œ ,|?ïnMÀœ AGN3FGL J1617.7-7717@s–¿šÏúÀ2Ûú Âî'À8ª$[ÿÛÀ;b!¯é?÷whlP
Y@m¼Æð?@LŒX¦¿âËo2F¿çFMqj,¿ëϋó¿íA1×8AGNfsrq?謁Öyb±?~ª!ø"?}ü	…"?z,'ˆ9®¥?k#1ãþ?ed†¯Š†Q?îLcöŸ"?¬k2þÚæì?ceXˆý÷?K²AAz?£
åw¼Æ?¨&¨™
n?íÝù» Þ?œÙë2,fÕ?¦"þ¬Ó9!?–rléi8ô?—Ë0…ýÝ?Š;p9;?ìê©ój+©?©YH]?¥	{Ýí?›ž›;NB€?¬:WJܡ?¥Õ9@´P?ïÍ£"o8G?s^é‰äÍ?sâvd°¸«?qxû˜ôÏ?U.ýñÁN™?N«nºˆÖ?ïS!uE§T?"‡.'LŽÈ?}ÉiÕÙ~H?w'îZ«?ŒRíÒo½Â?«G»R£?îe:FDTe?'­E°Ô¼?¢\x%%Šp?-ÿeÒ÷ò??Óu"þ?zš¥9ã4?îû•S'x?±Ä««?"ç^Éd
?'ZČ)v?‰þÍ7ò-Ü?ˆÚüÉkAGN3FGL J1617.8+5137@Sûݿη‰@F>'_ÀYøÀ9ÈÉu)wÉÀ;ýåÑ÷?åÏòª""B@‰Ð2
@—'ÀŽP¿æˆAÁ!¿é¿˜ð°¿ïÛÛ3©
?ékpˆB AGNfsrq?ïþS}´v?,we…ºàÇ?CZȑÚÇ?Ù['üSg?Lc? 쫒ãú?ïÁ»#¬'?~Î$(²?kŠ-7î,?r®õ¥å?q]Z9Œ‡›?s–'˜‹#£?ï×ã¬7V?ŠQ«QI·?ƒiåÜD7]?y¯OvPbp?"Иv—?†Í²iº{?ïð&‰Š5?l5¨Ø´5?"`ã.¤KÉ?:¾xm D?]fÐjÐQ;?k‰Ú£"Ý?ïÿ"å
í?$m
?óq&?
~ÿi¤?Ó¤©^?
þêšÜ?¦hÍÔ?ïè¼ôßÝÃ?df
½Ez?Uk/‰Ÿ¹?V…hõ¸Úw?Yç0'‡?W…‹ÜHì?ïƒ(ú}½¤?~v® ?u«/d5Ðm?h ÂôV ?"`)¦Ž"ï?{i]%ÇÓ$?ïþÏ6®?A&!oó£>õJý'²À1?;µLUš? e¯7Š¸°?=z'æü´«AGN3FGL J1620.8-4928@tÞUùµc?Ø°ä_¡·\À6o'£+ÓÀ9·i$†È@þÊéG×°@
*Õô"»3?ÿ´>%–c¿Íóê:zG¿ß7åKÁ¿âƲ†@¿ëÈMt…–‹PSRPSR?8T{AÊ?@à#lL©a?ì£+YJ?½Í	™Âðf?ºË²+Çë"?½½84"?%
i<ù?>2'{jL?ëL"ªœB¹?³@°>?ÂÊ2¼skæ?³LBÒ!E?yÂET?x'¯
•=h?êS˜•±ƒ?³êØ3?Åã‹úŽjÖ?³½é=cå?W|9·[ÌZ?U–PªÍ?è>navVb?¶ñ2G©L?Î×NA_=?¶ù¢Ü'M?æ€àÉ>??#ð/â‡5?삾7wW?Àçù°Òè'?»â¥²	[?Àå֘{†?H´ÜS;SC?f#g±M–?ëGÐLØH?ªI¨«àb?ÂÈ	󸍿?ª5̖vBŠ?"`‹ÀøÁ?‡l!v±Þ?é塸?±õcûWBÀ?ȵö˽œó?±~â~ÒÓS?WJS0Œ¹?SOüËwÍ?èr*-¿Æ?°X€Ñv«?͐0À£Yó?°q}œ%¤PSR3FGL J1621.1-2331@v'Àa"@2fþ?5ŸõÀ9*Et~WÀ;+Ÿé>ó[?úxÏ>ìúÀ@:Lj'Ä8@¥e;C"¿Þ¶a$vñ"¿éÆ»£"©ó¿ì¸ï6übß¿ÞÒ¶õä·êAGNagn?çЯà$dÜ?Äs9óì¡S?Ì:"ü Í?ÄëÓçâí?¢»§ÅÞ?¡üDÓ|eí?í&Nâáü?Âõ$,¸£S?¦4"Sý§7?²/J1¾?§f›ACÕ?¸°65ÁÔ?ä>6†ú°‹?´/ØDVˆ?˚)úþ†?°9á Œ?Ãlüá?O?°#9K=Ož?ßòhÃ
w?™9ºg0?ÐW©f¸"&?ǝíàØ?ÏkÛ¬tÎÅ?¼ôŠã›?ê$£ã@ùè?Ãؼ'…^'?Å;{ƒPyb?Ã5ý"'%?'§'"a÷?"£¢+ðf?îޜ˜†?±¢&Þu?"'é1¤–?¦2›=ö•$?4ÊéÆù;?£MÓÌ+£?çnY$?²wuæe?ÆNAóP«O?«eÕ­'2L?º›#åëàA?¨v¬eÁS?æZ¸³:T?º®m"E}?Ì(ŽOʪ?»E©5 ¦Ç?µéH±ß1?¢ÑÒ@
NfAGN3FGL J1622.9-0312@%"¿ª¥[@>¶ÌŸóPÀ9PAÌS*IÀ;cÊõ\8?ê ¨ÍFÍÍ@
Ãt±­·‰@ß@QSÛ¿Éxà^*X¿æ4ˆ1ߘy¿Ýx(ïý\¿ìâ.w¦nƒPSRpsr?çìùÇy?'{§/>?ÈMyЦv!?ÀĊw¡f?°"xóP?¨jùªó«€?ᬻÆ{`/?Çæâ'sõ?Ö_/@ñs?Äîà>ˆ?¹dÅË}w?¸{ìðº¯í?æ·-=GU¡?³˜gTï?É2bpìý?°_åÀÝ:?·áÑ4[>z? fÐcm(F?Ý7Äà;B?´›úҙ•h?Ónâ5êž?¹^ø<t÷å?Ïe˜yø®A?°¤ÊÄò©N?ë5¿Ó±æ?ºI§"Ø9'?½ðÀ"Q¨Œ?·tx7t5‡? ÂŽÎm‡?˜"aÚ;Ó?è¼[}ª$×?½&…é7?Æà"
R?¹Fƒº7³p?¬ÅÙÝdF?©°OÚÜû†?êÁ"8}å?¬LUC(s½?Á¹=iÔR?§‡®w±™>?¨ø6ߚm?"¤/?uÆ2?æ9Aü5?¦<n)Û?Ël¡k›Å?¦mû?­¾4?¸´óÍq?˜wBµ¡¥AGN3FGL J1625.0+5651@U¦J`"@EÿÝÑÀ:•é ÀièÀ<­2ӑ㿷@X»§S@"x´q·'@+¾aO?ïýØ¢1Ýb¿ê«»ú¹çd¿àgªÝtöÞ¿ç³Îߪ'ºAGNbll?ïDÝ¥?¾ëaD_ø°?"^q‡?¿¡C9Ä%?hmþæ›o#?mW¥ü¦ö¤?î£s?ÆG*?©³dÕnfM?–0">K? ±Œ
Œa?•vgí"xh? ï"ÎfHí?폣£§¡?šÙº¿?Ÿx_¯Ši?'&Ìñ«kŽ?§IŸQg?'€‹oùý?ì­¬rSx?®2OåCܼ?£Y¸WDÁm?˜À¢g¶'?°åÀCŽ?©^r—›>?ï*5¾ÜR?Ã5ÈTÔ(ó?™ÜÀ%m¤~?Ã:FÓ_I?Kÿ$ªjB?O'¥OºÖ®?ï©p]¤å—?‰!U°Î£î?wX•Æþ¼?ƒ?‡H?sï<8Âu¥?xCÑ8ãù?îàÚy™Û?Žÿk!ål§?f>KµÎ?†{åõ)òŸ?"~rz/–Ó?……c…4?ïgå¯?†ÝÕޙS?ª'ɯY?oNºÒ",?""÷Âd?'¥Xæ]YAGN3FGL J1625.7-2527@vP +"@0Ri¿·:"À6ñ\°Úþ¿À:u6xbm@O( °z@ðõ£ÒM@ÑBG£,À¿ßVàßØ¿å!¥øÞ´½¿æKf©¾f¿è«ÁYŸðAGNfsrq?ïצp¨ÅÃ?lµÎÉö/|?ZãáíŽ?_ÑäE-Áb?j瞐Ë~?gîxêߟ?ï"Óÿq?Ž=F–ï?r	5ð:-?}#>–3?'9o"}$?ˆW" K®?êf	"­BÞ?±cÔþ®ù?¶4³ûØn?¦Vë'¹~þ?¶›í¬†?¦ZM…Ô?ïaÓÖ<žR?"Èû€Cq?]œ8žl¾ ?jέ΋
?'ëÁ¯KØ?"0‹w½²Æ?ïìúHtÒª?^•Î:ˆA?Js5a‡PF?PÃÙ¯ña7?XÑÓéú?Uâ59©·!?ïÕóŸtyú?vÆ‡
{?]ª¯Å˜¹"?W4ê!*Iæ?k7‰@õ?sk©€qFk?êÁÁTYÚ£?°&_!?·"ö
Üóy?¦ï˜¨ÓªT?²ÎÿTyøì?¥à4Å3?ïËKÆÒã?zlÑi™¦?^á@GÇ?d‡-U؊?r¼'î0×?vÐ+ó—AGN3FGL J1625.9+4125@Pa¾À//˜@F@`B_÷À9Õ¢"›À;Îï@4£¿Ïk¶g/º@'G¡)Zí@›ŠË<T¿äoG¬DŸ ¿éÔìò9Ì]¿â›i+Mò¸¿ïùÿ•¡èHAGNfsrq?ïñ9!¿?XÓ>'R¬?Cö}e4?D@Øà_IØ?S'½O]ã™?S[€[i?îõ£J]? 7'ù1?'¿—û¡Ü?ŠýÖÅø?1×7òh?–ˆÿ=ngÀ?ïPIC–?ƒ•2"…D²?ŽŽœYu9?xŠZçv)$?ŒbTÅAM?xI¹ù©9?íÚàÚ(ˆ"?¢'?´³Ö?™ÇAêÓjm?'f†<‡ª5?¥nQezž?›S2(²€å?ïøÔ}£ÍX?Cn9Ô´Q?84ÁÐ?4ì»ûА?@"¨¢êU?94&›ó´?ï°Êô8)E?yK¹Ûȗ?tوPªÀ?n_L+%Âb?rÀý—`%z?q?€
vt?ïgóŠ·å›?ziM¸B?†µ2ɉ?po2ÈѬ?ôÐS?o8?pwݵ9÷Š?ï—ØÏ9Ž—?zü!µA?u'éò+:?g)[ÈmŒ‰?pšBÉ?wT3àä{$AGN3FGL J1626.0-2951@uÌó S\ž@*¢:Þù;À8>þ½	á*À:×Eßaô?÷¦g½ÿT‰@ Wš»-@IA½d¤ð¿ÜÕäÎ _¿è' +ø	¿äˆ=H,a¿ï	â.*W9AGNFSRQ?îü/êm?°ÀvÑÑ@?"ê€Zæýç?™šYäÌ«?šÿ¥úìi?«]´ÌÏ?ä|ø#<Æ?Ç?üÏôÊm?ʀ"®¿µQ?¾Í54a¨ß?Ã=‡p³W—?Àfjq|³Ê?çvÕ"õÎ?±êD×ËXƒ?À‹"N½8–?§ê±˜æW?Á™´¶ð0?¨Üem®^l?ÛÁwY(?³FÓ!a¸?ÑáWã¶?·ûtiA3½?Óæå'Ác?´麍<æ?ïŽÓ¼‰?­za³ە?€9K"•±'?ž*u GÛý?x‡eóÙ6?!A$TÌu?çþïÎsZ?ÁÞq
À^'?ÄÁ­Á¼ï?·ÃO
)N®?¹ü¬ùÈ®Z?¶–F•õý?éúÊ+Äæ?­ï9'KÅè?¸ykŸâé?£5·B³%?¸6tKÐe?¤Òß"½ó?ã‡C‹ê?ªéÇ+
¥?쳧.O?ª8˜fD¬?Ã&?òU¿Ç?¡ô†™CAGN3FGL J1626.1+3512@Lr"_õI@EôŸëWÒÀ:ۃ6€ÅÀ;ôyŽaW3¿èb‡Žv8@|¼êº?û2ýáAÎ׿ïÿ2Ìʸ9?ïýíXTø!¿Âs,·1ô´¿àÅÙ=žqAGNbll?ï÷Šã?ÍB?T" e¯•?9ø>Š»?K¼eœÝ{?Dòí ê_G?Jή§²?ïqÁþ?ŒÓÆ&š'v?yÆGÖ»"?ƒb(3Ô6?€×
güy?'@å;ñ*J?îÂ_ô1j±?'"K‹u'Ê?'Tؤ2?ŠÐÈ
ï?–_ü{!o£?…^[ÍR¦
?ïžò}zC?"šuŒŸ
G?rëa6uÄ?xà7!"99?~¥w€Ö?~J¡ËTš<?ïù3À?`!ÓÃð²ì?'|øÂàá?%ÿh®±ŠÚ?ET²×±s²?`½]?ïÛ3ÒëIå?lïëH|ë?`'ölÃI¯?Y(1Ò~ö'?d:6z—ù?fD'ïñ,?ïam"ÿE?'|+Ð`{¦?'©|/
b?}œ¹Ãù?"û#v¼E?t8z업?ïìår¤Ñö?Xu.)¯ä?NBþKf-?FµØ	å»r?W.÷Qj?Qû-ŒmõœAGN3FGL J1626.4-7640@s¤*ÿójÆÀ2Î_¿ƒ8.À9ÜKŸ:ÃJÀ;'"e'¿ùS)ÃGèÍ@+è«ûpú?ÿØJ^Èã3¿éI4'ª-¿ÔNd8Üü¿â‹&9O­¿×òÕÒ|["AGNbcu?ïï@_£\?Uvv#Ô¹?B.+U`s?=Ž¤«A?XhÛWraU?RC‰¦¤?ïvÈÄTƒ:?Y¦bËiZ?oÀlFn13?~•Þö.hÉ?Š]³à"Ý(?ˆ55¾i6ï?îèjVØKS?ˆ@¼›—Å?Šx–U¯A?{›ܙ" ?•¶iýØZ
?Z+_?‹["?ÝÒ¢ßqu?!v%VþZp?"ãîòʯ'?ŒÖD‡ÓÐJ?ǐwÜÛc?ïùbÉg¬P?@Ó¹òÀú™?.?@F¾î¤?%²^©Ã—?Bå	›M.?;ƒ"í?ïÓ½@V¡?pÕÒHÑnâ?W‰³þÖ×?U—Iëy?p>ò¶ð²O?jfã¿¥˜f?'5£ü?t
BÀA=«?yý麬?kk{FBê–?€–²Í‡Þ·?i[ŝ^m?ïæ/££‰?[–ïºr`$>þe«È;r>øvéùz?i"2rà ?[€æËÆ AGN3FGL J1628.0-3203@u·(€QÉ÷@'½ ‡_À9"éû±¼¦À;<êºô]5?û"á·©°@a&xº¦Ú?û ¤†_¿ÀñÒQ{Y¿Þ‹·½"k¿ë"Ú±¿ïÿexª¶¢PSRpsr?ž?#	";? .!w?îšÓсp?¥žë"q4
?ŒÌŗ®šÎ?'o+åi¯O?˜á+w©º? ´ÃöÍAá?ê'XMÉâ?¿séB	¡?Ÿ­1{³?¾´mUDo?°»râi¤Ü?›ŠdŠ}£Ã?êt›)Þî?«Ÿái3l¶?¾èE#J³?¥(¥É†O?«Bߘi^b?™Tƒ"\Ž'?ëå, m?±ÑÉ=¤è?ºf͔ré?«û/,ZªZ?À|¿Â7??¾(üxŒØ?ë]Œâj݈?¿F/yÀ5e?hk(‹ó?Ý¸=¯Ê?²ôÔq¿ˆ?¯XTQ?è¢"°Ô}?¿`a):¶à?ÄmúÖÁÇ?¼ÐJcY]?Êuåô;&?±ç­Vm~?åÝ'u]Ð?³^¥ÔoÁJ?¼-½¨l›4?¢Í¿O±z(?Â߁KUO#?¢§H?äæ?èj$—A®)?«B»™!8Z?¶ïدGðs?¡…ºbGPSR3FGL J1628.2+7703@[×6&-@A(?º*3À:†±Ö§A"À<bf&¥†À‹@€MÃ,@Í¡²—ÂT@—Á_±@¿áàð|¬,¿ç`Çk¿åšãˆG"¿â3 C+ù®AGNbcu?ïÏt§L/?{lߐ?\­¹¯Úë?h(¬Kiâ$?qkYýp?w"EVǦ?ï©×¬q/?sFÄkœŠ?r9­ù¨?'«ºwqØ?x÷ðhÿ ?ˆGJ)_mû?îVoú8ì?"ø·–ÞÑ?—"	àé	O?Žd@ÇEy\?šèð¡D?†ºàDÚ¼?ïÔVÓe1!?uӓ*^·<?."¹z¼Ñ?õ—§í"?uÜ°ÈÓ?uªÅ'N'R?ïòµ. |b?dk™¸²S?3?'xOõ?B'–J;?UÅÁž%å?c!7[}?ïã³|ªÜž?méÖä£ç$?XëvîSž?Y•ä	R¯½?_­Ñ¶ïÕ?eTê$ºâ?ï[\!û?}ˆw‹¼\?ƒ±ù¸l[\?v˜_^ì"Ì?…†/C4i0?n‡»ÇÖÃ?ïúQI¨?CËZånâ>ÖØâ>¨µÃ>ᡐ(:¾?F)[úÞ7?C½ú)DâAGN3FGL J1628.9-4852@tô	`0Â@¿Â±Ð ƒÀ8#ÙìpCÀ9ð¿UK?ø/L>h@ÝéÀ"š_?ùw/É~?ïù•‹–¢¿â3,}6¿ç…sq礿îA¼}Ê0:OTHERspp?buëÁ9Æ?a"#/Ô]?éã#È©sú?Æ%N–ïxÒ?È)™-°^Ï?ƍ…<j?Ru5Þ<™?oötƒ8ï?ۃ'¨³µF?ÃÑ^JÖ_?â5 Ëýo?Ãä´ñ^?£îZošê?•Ñù}î?àó°CÝ®?µÊýQÀ`/?ۜQ dB?´?ãQŸ?"$±ŒÀÈQ?wöÓþ½?ÖjÛÅQó?Ár~àä9"?ä1lË.?Â$©ø·aV?O/ù` »ù?NED0‹›h?éau¥Àæ²?È(,a/?ÊZùo[ò3?È%Èc½?k
'†d?R;z?7T?àjµ¿PH©?ÀVš°3Ó±?Þô€V7ÖA?À©6ÁCgð?³æ¶f±Ù?¡ìßM??Þ­íÞDÈ?³§»m5?ÜXdˆÉEa?³‡¯ylã?—}w«Ü]?—<̺oÇ?Ô_ÄÐmÛ?¶¤g2Q&‡?åD¬1Ì«À?¹4ªT…pöMIXED3FGL J1630.2+3733@NŸ C×Æ@E¥IÿþRÀ9´ s¨nIÀ;Ÿ0¡ˆ{d?úxuz*"|@©°Û.d?ôÅ›À?Þ,ôæØwâ¿Ü£9~Y׿àl³Ã¢'οïÿëÙ¾ˆøPSRPSR?{¶†n¬w?™u¨¥&ö?æGrN•Ô?Ï2çw·¶T?Òi_ûZv?Ïb'î§?µÂô~§ß?Ã~ÓàkÄ?êvâ¾cë?ÊÛ'û¾õ?¶…õôI?»…2%äb?´×d_¸è¸?£žBã¹Õ"?é¤ëFVóÏ?¯
€K]Ú?¾AoGFÍ?§ðG©¡te?§wrþ$^?²	à4¥Òw?èkö™àød?ºi,üjþ?·Q\M©!?ªÚ<dà?œ
€1t´`?¤˜"sàƒ€?å™ÑTÏn?ΫÈ\òì"?Ó
Yc.à?ίv&ð&;?Ærç.oL?ÏWn\^?çÐÝS¾Õ$?Ðë•ÿu~?´"ߐ<ÜQ?²NQÕÊGB?Ç1ƒŸvL?­_µ²#à?æuõ¨8Bè?±1¼8œ»?½íKQ¼-?¥yÒ'D?Ñ!í¾½s?°«…Â[¶ˆ?åúÊBü o?³€'ã+?§CíÛ.G8?™òãcœo}PSR3FGL J1630.6+8232@\ó(^ÃÚ¶@?@*@EjmÀ9<¿"ÀiÀ;¹½îãx
?ö*6ÊÂ[…@I¬3$E?þ9[-£&`¿ÒmOÄcq¿¿å¶3ƒ:2¿ä|1Ën™¿çÜŒ{›AGNrdg?ë±M>¼?·!aü(ÂÝ?º#,™ªÐ=?´*T5ûÿ.? ©UÔf×Í?$àå&˜˜?åõ(¼j\ž?È>}x?›?Íú5KÍo?ÅÏëvlT?´bƒ±9™5?¶{?W×øè?é4?üUŒ¶?²ƒü¶ÍƘ?ùOõ-6?®²óïèP?­×¢üŠMÎ?›¬A¤Ö‡¸?ápûV^A»?¸°S Í%É?Õ¬ž¨ò?¸³ï:Ñ0?½ÅªªÊ)À?®)Žl/w>?îK²l4—È?©)åùæØ´?§vù¨_?§vXß°£M?~nü A®í?{ýš`ÆÍ?뵟3·g‹?ºt"ßBÀ?¸=¬ ~Ýx?¶9	îJ³É?¤*³…Cš`?¨5ûs*#}?ìsˆåä˜=?¥ï²õX?µ<››œ‡?¢hj–"Ú?œœuþ†G?ów á½?èöYÈ7‹?«j[5Ø?w?Çø%5n¡É?¥å>˜? ¹Î®©j*?–Ül¤"^AGN3FGL J1630.7+5222@TÒÿ" @E2_×ÖìÀ9?¡F6E6À;'úÀûÞ2?àáøÆ®XK@'uiŽŽú?ÿæü9¢¿àí7[¿w¿Ú#{£¬\¿á¬ž=1'¯¿ß6"›¹ë…AGNbll?ïû!g"õ×?884³ë!?1úbʯBD?,烟i`?4úbG¢õÇ?/		á'?ï'õÄ£ïš?º´·i?yˆ§Ñ77?v\6‡/š‡?'~:ðÐ7ê?#Iò¶?ït-Æ–l?P"‰m(¯?}É%
Û©Â?töÃøß?"
« )?uÖ4öpûç?îˆÍ8NóP?–jýàý¨?†àÞöœ´>?~Ëô‹àÿ?¡ºô¹úü?"Ì†úÝ6?ïýBÍsÕ?(É?ò"Òm?&°t€ilÚ?!Šk«œ'D?%"°¤t»é?)E_¦Û?ïÕ*
'J?r¨i'0c?cŸÃx¾ïF?a"»Õä?g6/VŽÉ?lÎÓüƒ¬?ï¹ug5CY?oòG˽£z?qli0Uh?idS®×-?rAà;B?`ËBsÃø7?硫þqEÏ?stsn³?r]|V'A?YïâµD+?yÛiºbv?p°"Ä[ÝAGN3FGL J1630.8+1047@:uxmži@B/ÿ¢/À9›ÉØ)øÀ;†™°?ÎL?ár'3Ô÷F@éFÅâ!ô@o¬ÙO¿â"¬5[47¿íÕ=}µ¿â6}g߸7¿åÙEìüË¡AGNbcu?ïïëdp ?b&Hï~Í?G‰ûäh¯Õ?E¨H(;?V+*ÕÞoÀ?_1Î[¦š?îӚþù?¥?Kï®?"ÊòÒÑæÀ?‡	ýh?ÁÉ«³Œ/?˜ëÐ$ƒÈ?ÜÖ¨?—ž	#åï?‹§m‰ôŸŸ?x=†\ž¼?§ÚœŽÙ† ?–
¾$U"H?ê¥,$K8ã?¯&)E°?ª%8Í•?žûÖC¦Åh?½ÄÓé?©ì=ì¤Íb?ïøjúZ5?Kå«ïFD>?3K*8²ès?1'Ëۚ?D²*°(•?F{š!ù'à?cÙX?Œiœ
Ø©Ñ?{îVZå´¼?"
ÄhÊû¯?w¾xïϜ?€^Á.óƒQ?îÙ*sqä?•h­o/§?wÈ÷cLù&?b7¡ÙæZ!?žès¼þ2&?•o4n±3u?îgµ,-k¯?i¢+÷E?™ÔNîœø–?Íf´É)?™5Üû|?‡'†½~8AGN3FGL J1632.4-4820@uŸà·ö¿ÉA×ép-À8Bî'sÀ9æŸÐë??ø‹9L&õ@<öùñóù?ø5^ɹòÕ¿íù"ýW`?Óø/ª´ì¿åJ#ËÈQ#¿ê4zý2nPSRpsr?uù"žLq?™(o«v ?՛S8¥þ?Ð#8ƒ?åE˪ý‰?Ðk@.³?¥:³Ô/!?¸0ï)¹¤á?Ôdêg‰Éd?ÄØ!ê‹y›?ä{— ԝ?Ç@H&ÁX?µR‹á´¶7?¢2æÊ–?ڕ6ŒÈ¿'?·Žñé\'?à=ŽDÁ?·z#škÈ?±»ÍßO?®ñ"BzAó?ØïIñ³?Å8vk8ªŽ?áϟaüí?ÈAr]Œð`?hГÆ8æ~?pÁø£4`ü?׎DÖ«N?ÑGÓTa'R?ä 
"óS?ÑUf£;ó?¹t¢£µO£?ÂÊêv£AÛ?×Y€,"º?Â=°"õÚ|?áC>ë<o?ƉøÃ0ýà?Âêr?§±\êÜ?Õz€áß%?²"ÐÏ>UÌ?à¢Å3ì¹?²‰;FøÃé?±ï""ya?°ÜBþ°´?Õ3h7Kò?»Z?·i?ã6sÇ¢ìT?ÁׇÙÜ2yOTHER3FGL J1633.0-4746e@uGñQç?¾ó@`å•hÀ6°\S½íÀ9aÓÚÞ?ç	÷¹EÃ@ì!´@â¯3+¦?¿§¾åi¿ãg´¯Ÿ•\¿ãvt€Û\³¿ã†.þE?ÐOTHERPWN?ˆU<SŠš?Œæ˜°"˜?cçoùÒ?oŒW‡ÌÎ?'Eþ?ü˜¥$}"?·øQ½Xx?Ä8éF'E?¾O'úÄö?½ï3˜?é7hÙ÷ò?Ç¡h°m›?¹/¡ÛSð?§»7ÞÚ?®Å$-y
r?ž1"ç˜Æ"?êí¹ôê×?­`ׅÚÂ?°ÉjÞïYØ?¬'"…½×'?œ)]Õã±?–§PŒ@‡Þ?퇵°?g?°0at¶¡—?‰v•ï§(Š?V´‰ãWÎ?p(ӊãg©?€‡Eq2Ï	?ïyÔttF?"°ìkÂ?ÊÛ»ó5Â/?ÐlvT‰ÞÕ?»w1\;?¾a•'në×?äÆ"%f8f?Ï̙µö"?Àº²rG^þ?«C÷6
ö;?³¨!Ÿ5[?¢JLÒ²
0?é\SŒ¸5?°C]kέ?´nÊá­?¶?!>nC¸?"söÉÎ2?‰úi×ÎÍG?ì·×Ëë?·–mç¥p[OTHER3FGL J1635.2+3809@NŽ?é$@E+uÞÝqÀ6°"T"—À:¬Ò['@ä–ü±A@z®ž@©š¶$>Ï¿á\¿Uڗ¿æۋV`Ë¿çË,æÃ¿ë+ômáÁAGNFSRQ?ïÁÐ(±­?~½fW–͉?{ñ]À@¤?~NÅëɝ?I4qO7Ež?HÀàûªƒ?ﶕBÇк?‰ª»B]£?roD©Ð»?"
š¥.Œ?rœïlz]?wI{À¯?éMP©¡à¡?°¢`ݜp?½Qùê3²?§Ñžûz¬'?¸†(¹â®C?¦"ü!ÐÀ?ïÑt¶Ø'?Ú"")Ë´?I\¤³11?fä"7¹?tÿ‡??€#žËF·¸?ïɂª^?‡øRۛÒ?v"v¾ž³?'Á1ˆ˜%_?RéùœyHò?z|<þmÍ?ïäòDDlZ?eu<²ØÃÈ?WÖÝ؜éw?U;1xUΪ?^D™m
?\ÖbÅÃ~O?êv£XgÓ¬?®.ÎS{³?»(bݒ9?¨—f[Ê?±"àÚQÃã?¢ÍÏu+x?ïö¾@ÿ	ò?\ ¡·}‹Ã?7Ö¾èÔ§œ?Bä(³_õb?I›ÏÅ3?Z*'èV°ÜAGN3FGL J1636.2-4709c@ubŸœèÙ?ÀèÏÀOÄlÀ7f×süPÀ9‡ëÕ¦"?ô"Þ+ÄÔÜ@4ýOü@·˜?§_Ö¿çñ¡B…a¿å©î{s>¿ç¢8¤Œ;ã¿èW}?pÙ1OTHERsppt?zZÞêÜ´?|'XJê;?¸;Bqê?¿+†
7?ìÃáó"Pž?¿"x1an?—õ0•µc™?¡"ˆ+´Ãÿ?Ä·õdÆ~)?¹Eÿ'bÑy?êY"Ið©?½4âéL?±kö'Iòp?›K‰Z !?ÓsÝó:ʬ?»žÀ0By3?ä'49\\?»…h6D­?¨7ܑñŸ?«ö‰aL§ø?³Vtèˋ"?¤Þ¤E,t?ì³™þvò?µÒ_{0Y?rƒ½œP«±?ušŽÿéÛ?»ï-ásÅ?ÁÓÔ0¡ç?ì]ä¢ñ ?ÁoÑ8CÐ?¬%+(d݁?±(¹"o?Ìwø9?¿žéuáè?籬ñ÷:?Ä"Ú;†z?·t/@¤#Ð?¡B"`Ád?Ó²åáàt?µaý0æÔj?ã8w$ú‹L?µu°TßÅ?©±^'"vÑ?°ý¥9Ó?¹hGïþŒ?¤4¦"ƒm?ë7箶r?¸áξHãdOTHER3FGL J1636.2-4734@u{à~í¿ÄC€³CºÀ6ä'eîqbÀ9'!àÄÑ@=ÃòI´@ž>ïÔå?ûC¼˜L=?­Müƒ"À¿â8¶)ó'¿ãþÒ–³5¿ìö( ­9OTHERsnr@?6ʐ=ûè?0.R¾,Ê?êÚ½ÄNׇ?©ŸÚó£?ĉ£¦Ò?¦='˜Ú"?9jÇW»Ë?Z°p1S§¢?å
=x[†?¼Ý"'/ùÔ?ÕßlÓy?¼Úh×.ûk?{ÕÁN?u'JÌò¬n?èkºú‰?¶b¦®Ï¢?ÍxӈJ3L?¶7	(ñÜ?w}@ˆ ??sÎ~?+}?ÝpÕÔøK?½›X幯?áš•k:?¾>MYhì?#'¡íÇ<I?!Fèdwã?ì(‹_@?Àü^'9?¾±ã´½-ë?Àƽ^è?Pм€W]õ?h¥PÜçL*?ç£S!˜´ ?°Ýßü"?Ш‰o;¢?°IU~`?}J'•´r¼?þì"id?è»qø7V?²ñ¤)Œã ?Ì)5¬<çð?²Ö{áȓt?rßd…äѓ?r§Ž?Ät7?àS$ÂØ^?¶‹Üijñ?ß8çA?·(–ßà8MIXED3FGL J1636.7+2624@Fßß´0@D€C‡>À:FوœòÀ;Ú´*>—ë?áfà•'µ
@ñ‡î'ð@Pbà?êøì#eq¿âÅAµ?¿×-ɀ«Ñ¿ãÊ*î7¢üAGNbcu?ïß×Ó)÷å?o/~0|0'?GTÒö
?B­ÑÊ=Ü?jRø×VÜ?mÀÙJpÔ?î(§{Pû'?³L§…Ïê?Ÿ)¤T¿Ô?¥©|©ˆtå?›ÁlARÍÜ?§²<UUMä?îöؒ¹ç©?‡íó€CEö?‰a{ôVÏQ?yD.fCxŸ?"t/¬ßÕ:?€ÒÙþüÜG?êÿ¬·ÈGœ?¯õ1»{ü?°‡Û½<?£ÅYGZ¼?¸¸*7é?©ab¿*?ïõ­^G‰?T¯Wãý?1ü"­
C?-Ü{áŠo?P&",‰›Ï?Sj-)à¢b?ï`Öu~BŒ?Ÿ#¸–ßÕé?‡?4[Aé0?—¤Û:O'v?€‹.Qä©?Š×¿9ÔF›?ït\;ü@¿?yæøÒL.%?~9µÀÛÅ?r›a‡:?ƒÌªf?o2Ï:±Eú?îlqÈÇÆ?"ýLœ#?žâÄKèÛ?ˆ±s§'ëv?"ìãPn?Š	çMdèAGN3FGL J1637.1+1314@=ÿ¥ßøù|@AÙÚÿ•võÀ:HNäi¡"À;›üD}Þ?ÇÇ9‹£@§ºu\M‰@Ä¿Àéz¿ì/죛"à¿è˜É:.Û¿ÃÐ'Ü}¿Ñħl¥ÎAGNbll?ïð‰vЅ®?YÑð[ä›?;{݇·DQ?EÀ¥aár?Xs+ü?V4'Éá?ï—	©Ìí"?ˆœ§2aæ ?tNôêa?s¯#ª»;;?€k*E?"¿'*#9ø?îp)#B'å?'Õê×À??Žå—6ªñ?~äVC
?¡D(dRXö?Œ:òîjCz?î_<íL?žvn^fïw?m²;'O—ô?~OFã^÷—?¨1EȅA?œ'",Ĺ?ï÷«5€óä?R†˜bmD?0¡d$l]E?4€ï¼ÇҜ?Iw¬ôe#?P|®T!Ly?ïÙgæÁã?sö`Œ?`éå·¬`?a¬*ŽF›Å?e®˜iÐ̉?jÅCéQNe?ï`P÷ƒ›?}`Y[aã?}RÂÈüƒ€?m4díߦÍ?‰B`µ'í…?v˜ù`©Ž?ï›2õ19?xKF?hs£È	k?c*'[ç™ñ?ƒY¸Ìó`?sº!è­àAGN3FGL J1637.6-3449@u«•¿ðEx@ \îøœÀ9Qc"GÁÀ;"g¨…ŧ?ñWmû@
a–4à2?û¶¡>ÿo6¿ïÿ¿Ä.KK?ïÿ†ªBx¿ÛÓT"	•^¿Ò4>ñ'cÈAGNbcu?èh õ¥Ö`?Ã+V¿n.K?´ý'Ÿ¹Ë?­{Z";°?ÃÞ²Ùº¶?¿ã‹ïÑ£e?êóíKƒ??Ƶ‡M‰8?­l;¿ñ3?²–>ɨûÃ?¹ªŽ–Òj?¿äŒ
~¢â?ç͗úvíâ?³žÚq?¸°Ëi"Q?¡)Ž…‹½?Äq:aÈw?°ƒYÄ]
Ê?äـ³TçÊ?Á›Þ9Ôš?Ì\)rÙÖ?ÀèÒ¼ÐÖ?À=ñ_H?¹Î*+2ïÓ?ì"Q['Lô?¶Á&"ô²?«ÿªªïõt?¥¼û'ŽæÁ?°íŸÍ¶¦?¯èäo%³¶?íî'Ë&âö?¼þT!rôó?˜V.%ð|?©•Ãîy<N?¤ë¼B<a?²e©Ÿ?.?ìIëuѵ·?£Å^ÿ ÑË?©ÆqND?–gój?°ÍkÁ	Ä&?žw… ýáÏ?êo©e`ú8?­eÙ¼‰ª?¿/lÕp«?¨ㅝy¨?ª¦ÿÅ{'?žêq‹N vAGN3FGL J1637.7+4715@RYÉ`0Â@@DñCÀI0ËÀ8'滋[éÀ;ž{Àj¾»?äôÛìû@~@T7$Y{œ@ð°ÿç¬L¿ã{·¨<8"¿åæÞP$R¿ä
këØο谨Ýaø÷AGNfsrq?ïü¸
Ú	Ý?/:$¯©ú?)#6Žô#?$¹	Úrõ?+\'z7À?#!E¯–'?ï¶|"?ˆüUÜ=i?p&ˆ'Ó?'­{	wT?tËònáKí?x
cF<ã?ïig¸ x?y`!Èc›Û?{=	çݎÚ?h¾}'€?ˆÒì¨?r¾*sJ=O?ïñ'$Œ?c]ÐÅɱ?%‹máù½m?-ùÝbuÂ?[Ž`T b?b'»šCV?ïþ&z¬Þ?!O×Ú9'?!r&®­Œr?!ûC$?6ãA™Éª?ÀU^82?ïæEÛ<¸S?h…'â0Í?V'|nÕé‰?U+™jƒ"??\ñÍgp_`?aŸ(Î¥ø?ï­XÛ/Þa?oFn)š?pK(Ñ:.Í?[T"Cø?yi‹'ô?jÈÑë¯*?ïýмVÄ?:zÅAA?¿\…ïw?ë[{]ù?,U'NÍX?9´ïæAGN3FGL J1637.8+7325@Z~V>Ðö'@Aœé	:;À:è¢[ßú§À<<zØä2D¿¬'–°OÄ@ºðëeU?þ™é`+cÜ¿í]èK‹ø$¿¾­èlK¾Ö¿³a»Fg˜k¿çòג<rAGNbll?ïv6
("? A*áË›?rÜޖ7Š? (Ô[›U?HÌ:ÝÞhú?Es³;Ã
Å?îÀÍpò'? §ÙlP1Ý?"Èöæš_?"uÿ枒Ï?"[dè}|?•]u ­§?íÇ 	­U?¢í%)ç!?ªÛØLµ ?£Eç™@~?'dN¡2F"?yӊZO?x?ï(8¿þÌé?'€ª¥Ô'?‡3[ª©??‡UÖf͖+?Ž¾tcaö«?…ôºsü•?ïÉÒEee?'ØïíN¨?ycÈ §?'˜ uUí?;=œb?6MÕ¤û`(?ï­8ͦç`?{°D…òB?u¹!©-ðX?kوJ#~!?sªwvOÛ¿?sǃ÷˜À½?îdE:'îî?ŸÜI…pr?¥cPâdœ^? Ƣ҂?amØŒç?fÐ(
?ïÂĂGæ?qF•[¶z÷?tÎõRÉAÐ?hì‹lüËÍ?d]PÑF^ª?_ !Î$ôSAGN3FGL J1637.9+5719@U¨s¿ë<ú@D2Áð8À9ÎØuw{À;÷–uŸÀ

å@CsõÆN@p¸ßÚñ~¿êýiEÛ_¿æU¢å®×*¿ëñð¿åžo"r@AGNfsrq?ïþ¡Ç5Š?²L™&>¶?´õ}ç!?X£Ç*UÇ?àv•?^
~Δ?ﺧ¼z¢¼?˜"Ûl±?mX±CBß?q¹"±æ~?sÿÉ2;L?wÅ0"|:?ïA{¨lñ?ãب0_?'ûjc"?uúžèž?Œ¥øo	o?yiñÛ®ø¶?ïòD½8?]jZB©Ž?ðé-F"Ô?#eÔ­r?Zvþª6•(?\ð+橒ï?ïÿ-º€?,!TzB?~àW­ù˜?nr×J•?uÀ¢Þ=ƒ?s¢`¨ç^?ïçuZ¨ ¦?bá6	Ö_?V^϶Ÿ&?S"p»w
‰?Z¶{,ì$/?Xêµa€L?+•ô¸?pÈÕj°A?to4d
i"?chovΝ?z¹5ÓºêZ?hxöÒRõP?ïþz´"µ?63+·Ä{>ιv}æv'>íéʀb_´?.]q{yì?6#ºÒAoAGN3FGL J1638.6-4654@uƀ"?u©`À7W=¼ùðòÀ9¥ýò߆
?þp뽨@g¹X%ÛÝ?ü·2Ü¡+3?Ç1i™÷k¿Ý÷áìåLjar¶¬¿ê*r.ñ…OTHERspp?ƒág?%™?'卽
?β¡¡êÅ?Ê2Ss^`L?èÑúÅ>Ê?Êf9±~N?
''äqK?ÉÛígè?Îü:ÙDÕG?Àh$£ð¬ó?çü¼«0^±?À÷JöYŸ??¦g}b>?˜´¿3ô?Ô
œ´‰½Œ?»N˜:/7?ä"9Ԟ8¡?»ŠHX^eç?¥^'î•Û…?ŸË.zqò?Ê;"'8öc?³P°ú¤Ås?è5ÇHd¯?¶ó¶ŒnŽ?"ÆZ¶½"_?˜ì,.IN?Òå×4Ú¨-?мÝè?åîá|Š??Ðâ_I?'GÖÐç?žÁ
?×­è?×vÛÅÛ?¼òZK¿¶?ãê¸+;?¿VPüi??¦g¶—ˆ·?0?ÕÜß^ÿ?·"Œy]†?ã«øAÆ?¸"ý¼"¹?¥
b
8?¢'@F"@u?ѳ/zÊ?°ñ§Ö%ð?åÕÂ!֝?´Ñ|­ýOTHER3FGL J1639.8+4125@PdzøÞ¤@DÎ3_¨ÝÀ: ¸jßrÀ;ÃiÔ¯ð?à›{'=™@"NAxÆ@UÀâcb¿ãõ×|B	ª¿æϐnw¬à¿è¦˜!ˆˆ¿ïýžIè½AGNfsrq?ïðr0"Ý?]eMsšf?SØ!×¥Ÿ¶?Y^zã	Êæ?F†ü' Öý?BŽœ'~¼ƒ?í"0™[ ?²¥"Ӄd?§;®ñ3 ?¦/$h'¥4? Q•+b?§$B|?ï& $°
?'E:±©ž0?—D@%þÐ?{íÚÖ1?†à²†Mî?r
-[!D?éãäêX?­xózÄ=ó?ÀÀ*–ÆD?§\<‰ü¡.?°Àh†dh? ‰'iH»?ïøD§Ï½B?Jî)¬x¿)?Ft5U%?H³øØ%ë×?1½ÙË7°ß?*O™XXNº?ïJ´pN`z?–AV'Æ?‰ïèÓâ—?‹s÷ëÖʟ?ƒcâªdÔ?ŠÿoQë†×?ïk'	N՝?vkKÁ2.?‡Tä;a?qM½QGƒí?{ŽÍ'äV~?dKE¥
É?îh»¬O:?s]Ž´5?¡àžä‡)?ƒó·#@—?ŽNÞzî4†?'u&;^ÀøAGN3FGL J1640.4-4634c@u$_•'Í¿"'‹Ÿ«¸rÀ8Ø{,ÇÀ9Ñ)‹ê"n¿ö0	£—Ê@
jthÏ?ý»¯ÞÕbó?ì} ⣣´¿â:Áœíáð¿âNªRNm¿Ô½p"ý°ðOTHERspp ?'#ÙsÛ6J?œÃé¬ßû?x-6à·ôL?‰
9*$3?ï>†ÆX>…?¢³œƒ'—?Âç½åw"?Êùo:\?¨X®Ç%?¢@âq­?éÄZýžô?˸ßÝ\?ÁOѕo¤?¨©>U?¬:ßhʈ"?›:°?éè]¤nS?­¨\lFã?Ò=Áƒº×y?É7Ј»rT?RÄF^¦?[b»XՇó?æ×½=…?É;aÞtó{?'¨¿ùÀûÒ?œ"›öµ(?"¨£×óâß?"Výµ÷7?ïpßç?¦dŒÃí?Ђ'c,†W?ÔŽ5Ò
Ã?¯à£?öë"?¤J+MYѸ?åÀâ¼ÄÂ?ÓMøOÀ?È5S¿ÛÉ?­n–ÍÆ;?°…ßZF‡?œ¸Žôœkþ?çáï%^«©?°¹'j+‰?Õ7¾~''Ÿ?Ç5Üt¤[ƒ??F$ô?<b¬võ%?å`7üNMI?Ç7Hx¯OTHER3FGL J1640.6+3945@O¬Xߕ&m@D²•ÿ±%§À8æ…Ûv´À:"+,Ôta?øãW/ç¤?@6€´yS@5­ƒCl¿ÐbÜXŒ¿å~¯´ý¼ó¿ãÝtŽ-î¿êY©1<8AGNFSRQ?ï¢rÓ?‰œ"Me?c²¨ìðD%?cg^¿ñ§?''y.©Š?‡×y –=8?流Ïì?‡™ªØӍ©?s*X€	$?v"ìüKÔ?y^_ÖJÁ?€ˆ×5K³R?åcbR]?³VfD?¿#í'X÷?§¼§È3 ?Êà¯.ùŠ?±ØäË*½?íË
/âNr?ªxʨ@Œž?€	ù²ï»?ƒ\Æw™¤·?¯Lޔ›9?©¬>K^?ïÑ$ö¸R?{ÂAG¹Î&?Yƒ"Hø¼r?[Ï»xiXÁ?qŸäù÷£?yz]Nü?ïØëз׷?o‹»'ª?aÖwa³"´?Z¼"ïk?e=·® ?g?0Q·nË?çè3Þ²[?±D!E‰œØ?ºrÊ3%­u?¦êØÀ9Û?Ã%Ëk£½	?ª‡üA&?ï0=œ»™?‹(Y=ó{?8c'WK8?uɎ—›‡A?'*3ˆ­3?ˆ@0»—lÚAGN3FGL J1640.9+1142@<āŸ§Ð"@A–`)5ƒÀ:ÛeìÃãÀ;•ô©Š¨e¿âêz6Õn@Ív&wãç@]P¨¿äÌ®>0+¿æa†&(¿Ð­b…÷¿ëb$yµùAGNbcu?!Tþ#?ƒRøF/'?weFul(?q¶TÖÀg?}T(ø"
I?{;õuÌ®š?ïÆ/=Ÿ?™Ð.Ð#Τ?Œ7Ëè.$?…èÞ^?ŽÂ<nþâà?"œT½z'?ìük¡õÄÏ?Ÿ}–ŒR?¦½>Xc?"UuÈò?©|ŒŒ ý?"]踮?íéH·›?¤1ëq"ñ-?…vù&_Ð?ƒ9ñÖ®
\?´‰Ö•
óÓ?¢i|¥ªåj?ïÜƄU²?hw^+êt•?`šXÊ´&2?Wm1T3z€?bŸ#SCå?aÿn;C6Y?ﴄRÏI™?zÙåÊ)ÆV?rµM—›Ÿ?i‹7E¯i<?s‰©q÷?sÚζe'?î²oBFæ2?ˆBfÿSã?—"÷Ž%ú?…°e¼\&?'š'½ÝEÁ?| óÈÁ?ï8™\'L?'jÕS1"ó?q(¾°jn›?aIÜzdT?"¢¤Éè/Ä?€ÈœŽ>AGN3FGL J1641.1-4619c@u(; îÙ?®æ»Ÿù'À7'œh€òÚÀ9›œÈù¶¿ÏcôçH#/@
ešO±™@:_¢Qú¿åPŸŠtb¨¿ë%nâO¿Úÿf}›¿æ|Í{Hu»OTHERspp$?g‰"ÍÖt?xë¹q-CJ?uKžÜõôï?‡²`|üܳ?ï½Ë8çÁß?bÃ3,?±.C¹-?½Z@EóÝ»?´ñ'5€?¯sZ7%}Š?ë<å‡?
?ÂÀÍÆ?¾F§â»)??§…±ò`B?Á}‹¼6Q¡?¬´OÄ· -?ç×È›p?³*ý"­á?½CZ)¹"=?¿¶z"µs?y
5µ"áÆ?wíåG1ü?ì%€O›ž¬?¿÷{çþh?f§ÇÕ§?{|nvo?‹Æñuát?¤ÀˆŽâäð?ï}i<¯ˆÄ?§0#k6|5?ÄÈotEæÙ?ͺH¤J^?»éjMŒâ?®(=/<a?çmfõ¤Ô®?ÎZÏ%äãf?ijó¤ŸS?«ŽpQ¾çñ?Ã$sÔÛ[}?¬¿›5ûåi?æ	æ!¡T=?²£R¿óÿ?¼™:p‹¦?¼»¬ Ôô?}&E€éý'?p¸zñ:ýÆ?ìBM'¿¸?½/"½i'{OTHER3FGL J1641.8-0619@%¤rAeûÝ@9ÅYa›À8ÍÎ8׋À:æÃr°÷"ÀëýT©û@ˋo_^_@†î_ċ¶?ߟ'
ÈÊ£¿äeún#QÇ¿ãEk5œÞ·¿áÊÞ:ˆgAGNbll?ïÑÖ'z©{?t–=4ÚK?QxуXû?MÖõ»"q?r¶·ðC_Ö?s:]©;h°?ïžmq{ ?"I…ÿx?nwÉFLÃè?s"s"yÿM?€Æ±Dþ8?';[Ôù?í—‹Lq?¤5í|äß?›>í*Ú,?ÉéáM?°[ŒŽÉOø? ÿÁ&1Š??íøÇE¾?§2^^—¥?7––ÓavÁ?I²‹´ŒrO?°"/<Êñ?§'šp%¤L?ïéW|D'?p‹»xO;¹?D$'4T»ž?Tzåófÿ?aŸÖþ¶ ,?hüW6m.h?ïÞý}ˆ…º?l¹nÐ0??Z@!l…?V]Uû?câqý°ÞÇ?f—YsY?îüÉS4t@?'ƒZhog?ˆãêê|ݍ?ƒaŸ2"ê?"ôà+A:?Œ_Ė:?ïe¨E3n?‡ ‹E*ó?_«ïi?	жE@•?"BLÁÿ³7?‡Ҝ%­<AGN3FGL J1642.9+3950@OÀÍ_™Ã‹@DyvÀP½ˆÀ8"è1­!À:Á͐A+C¿ôÁ}ÿ	_û@;64D€8@"H?ß¾í¿å֜ƒÑ'È¿åÃT±¹Õ¿æ0'êðñ'¿æ‹Z˜
8´AGNFSRQ?ïø¼ÿ4Õ?Hƒ'ë7Á?-ãê[?+dvÜ͆¯?EÈÉóא9?EŽ(N2?ᆭ*ÃðR?~"7mԗ?m'érYÃ?p¥Çò"Õ?r*V¿ü(?u.R¿8¼>?îMf{ñ#?›ìÜ¡Pÿ?…gÔÊ	?‡ž²M¾¦y?¢ì…°Ë½Ã?•"³t`l?¶œy?ˆ?5£d™i?#M»û›*"?8›y¦ˆ•?‹ÊÇ!Ñh?ˆ1TЀ¥F?ïü¯y2yƒ?6Ê{¿^?%$»mæ5?-DϤD;1?/ã³H•"?.ñ/¸a¡w?ïçÖOÏÃo?c'øççÁ)?UŸ‰Xêãõ?SՀò¶?Z³×I†¾l?XÀ
;D×"?ï+ÚNjœ+?Ž¥žîÔñ?€‡XL
ôÜ?x;Ý2–òH?'A
	¹Õ3?‰Ç«æþEN?ïá
`ˆ"p?deéÿ»Ÿ>ýCk/֚¦?¤Ãâez?n¸•
.P?d_"EAGN3FGL J1643.6-0642@%"~e`­@8zE¿ý±qÀ9†ãOÆñÀ;…CÛ?™zVº@Ð@2*M±c»@'
 yó¿ìK1uT&.¿åw©Ò]'¿Ý|•DDº¿ÓÑýÀ¬ûCAGNbcu?ïãìV³s"?lÉåÃÿú?LGèѾŸW?LÅ÷r?e®èH›Ö?iÌÇ÷)ˆ?ï¡e›:X–?‰З,ð?p 9«¦A2?nÄxvӀÏ?~¬øśσ?…åªkjY?îL™"º\ˆ?œV431ö?"sáôÞ+?â]v¶gF?¡|uÉë!ö?"Òy—Ã?íi:ðۏ?£¡~7kã?aT:÷ù?d<NF«QO?·jDü,Ž?£,"P-Ö?ï÷ ^€z?R+ü`éó?8Ò¦B3²æ?=þg09K?G2ým-O?JÃºœe?ïÜJÏî%ž?nR|²¬²Ê?]Q[«b?U
ÅrˆÜ$?e'¬q?hÛ;‹{Õ?ïD]êŽK)?‡vPœÙÅ?ƒfÞy§?{òd—÷[€?‹åt¬œ£?$È­÷~?ïžL~*J?… s¥"™?]Oß-¥ê0?Rl![j?—8ƒc©?"»#ÐB7AGN3FGL J1645.2-5747@t£½ßÉÿ"À¨
`+8éÀ9–u—5À;Í#3᯿ör25J@
ÝeÌ7§@f+ —ºœ¿é7¤
zœ¿êäT®-${¿à.­i"¿ç^瘙ÙAGNbcu?ìJê+?º^µ¶
v>?wùȃAÐ?t€Y ;?¼/Â¥×j‹?¹ð
Cµav?í)›'åm?¼"_B'9L?'
*b)? sš§AÀ?²oCØ•?·|AÔ<¬?êjn
%Ô?«k¨Ð±B_?¨5×^?•0gùNæ?ÀOzpÔ\?¦}Hzú}?êUÄLö}Ë?¶Øƒ«+ùi?]°ÇĶd?[}я›¾3?Æm=&j?¶ÆÓ#)Á?îÛE{_Fâ?¤b	ôñ:2?jdŒ+ÒØ´?jßĜ·¼0? ¥_" ÀÓ?£ˆš‹	ˆ?ï=,Ó)¢?¤š¾PÀßD?s˦¢ç¯%?'vd›k?"g"žô? ŠWL)%?îZ¢X¸†w?'@{ζ£?'¾‰Ásù?€SiÚEM•?¡v•"½œ	?ŒDVy¼âý?î¿2/'?›õªkÂÔx?ER¡ÚÓ??~˄)TÓ?¯?ö£Öv~?›Ôaå¤êCAGN3FGL J1645.9-5420@tÏß֔ÍÀ'`óÀ9?‰i ­ŠÀ:æÂ:¢"=?î¨JG³3@Ȗœº
}@¸€nz\¿ÛŒ8óf"Š¿ìŠ!n«¿é3BL«ª=¿ïþNh†ÒOTHERspp?ÒÆ
æ¸Ü*?Ç[¶‡ï€´?ÈU«°>îö?ÁàµhhZn?à‡ "Ö.?Îjµ‹<´'?·h‹M´:?¼ó«³K?ÞJq'ànÀ?Ä%bbÿ1W?ÛÎ4µƒñ?ÅtìðH?ٙ°]Þàÿ?²ç¢›]Úu?Ñ2ÆÿáÕ¦?¯¬åÔ?8Î?Õ3ˆ¢?I[?³	€…ëJ?ÁÓ¢ð?©"6v[<l?Üebh]•?»…Ý1n?ڰ̋´S¯?ºd«G¹I…?ÎjH«O"?Æ|¶/¸'?ÁÒ½ìN@?»ø
 u0?ãð¾TA©K?ÌË €º5Ø?ÌÙ]Ý^s?È~hÐEu?Ú͇im,?Áþ3¬Õ¶€?×&4§ãš?Ã6Zº¶Ÿº?ä Â,à´?²nG×9â?ÇíâØ8!?§_FÀ{è?Ǘš\?«ÊL'E`‰?ѳסÉ2?°g¢ëÒ¸?ÚûC8 Æ?²¨üVó^?ÓPå&F!?¯‰Cª ÄMIXED3FGL J1645.9+6336@W‹ž_Ñ÷¯@Bó©?ÿÊPÀ9ÑaE•5‡À<5ŽWF8¿íÍ2Ñhà@kC¡•f"@|/@_k ¿æö~b—µû¿éÆVv·Êæ¿æ_o¯:jµ¿ê'æ½õՖAGNfsrq?ïýóBNÑl?*k íM"?}˜Ÿ²æ™?)÷Œj‡ƒ?$<XÇ?!Øx]r6Í?ï´Ç¬kG;?~ðñ±ëð^?oȅÛź¿?n;«½¶–ï?u·æÁ¬'{?v¥LTë2t?ï3^F‡Mè?†¹ÅºÞ—?"§X&V?wûÂro¢ê?ŽQÿE'Ï?'³ršÐq?ïÒx¶‡«?uDœá#{B?Fw'åº?G»ê£õ<8?sóÏ7»¤ ?t)JF36×?ïþ~¯Ã?"ÊËWø»(?¬kÿ–ç?wŽOÜRô?}­jʾ
?GH›pØ?ïâÃéA?fúS
.>ê?Ymv³`4?RâëÐN³¬?`…[a4)Q?a¬4ùÖ¡?Ì+DÛ?|íéMD*?~8ë'"•?rø
BÏ?~²`Þéº+?to¨ òÐ)?ïù걑T?NÒr.6?BA¸ôsA?"U=»€?F	
Lq+<?M€?±íâ•AGN3FGL J1647.1-6438@tOÞ²gÇÀ(Þg@€ùÀ9»†ÜþsÀ;•BâL'ÀxwRœÚí@Þ
ô¸@ƒÄ`Á
¿Ü€Õ$V˜à¿å.ߥRƈ¿ã½Kõ÷¾h¿Ýÿ¦ù¬ÕAGNbcu?ïøÁó³t?A©©ä̙è?àC›Øá?ݐJ#´?J([]Pæ?@…fÛìgÈ?ïy|·ÐU1?'M7¶è™c?nÁˆµ¥M?u{¹òC·?‰ð‹^f"i?ŽæF®U·n?ï,=,¨¡í?§—hÑ̀?Êý¿ó—?k«SZó?''ۍ¥‡ž?zÏYBëh?ïÏ0¡!g?uŽò4t>éÒÇƸÓ,?}óo?xZÅùgî"?u‡u쟇¼?ïû	«ƒ?6b#'?÷?KZç<²Ž?ÅþÝî‡Ô?=ìÛ›µ—?4I=¾:–?ïÔWš",?u¬÷çý¶?U/)&גž?Uìôàš?pˆhSWi>?q<€Yñ©Ì?ïªÜ%ôõû?hZ§¿—È?po"0Réì?SLE¨~­?z"Yö.X£?cŸò¨AeÆ?ïö¶<‰ës?Kì֋ƒ»>¬çŒÖÂH>¶ß\Ê·s?Rê7N]?KêÑØjÞÈAGN3FGL J1647.4+4950@S)®_ú;›@DvŸ™ÛÀ8¢ßüTÀ;±m«Õ€?ëO§Á‹·?@<yX@nÈáÉ¿ä»ôbgÿ¿æüÓ¦8l¿æ"ÑËAæ¿äð滜‰õAGNbcu?ïúÓï'á?<
Šþ-ˆ–?5n*ÿ¸?0n¨-)?3òZ@äYÛ?1ŸiøµÑ?ïfˆˆ'Î…?'ò™va›?J¹Ø@'Ù?€ƒo¢®wî?…#ü½?ŽP܊†¶?ïS,‡óSõ?¤[û7ž?€ÇY&ÍÍ?lN]D‡ä?Šm¿·j®Ø?xÊÐ]Lú–?î»ZI«"a?›žï¢m[V?Ž ¡¼!½?ƒ˜è¸ži#?™Deå«ù•?—´M­z?ïýæè¬Ò1?,X""÷[
?$l$À¥‰S? $Ôõó˜Â?JšÂT—3?!Á¶-Jÿ?ïÌÂpîO?pæ<0Çþ?i!ª¹ÃUä?`†j?GiO?jäø"«=?i´·y´?ï¢Ôì?q…Ì÷¹¤?usj»t²?fJòOâw?y"'Ì- ?fùhçîò?ソ—D!?y^eþ™óæ?qgIC¢z?_¨²U Ã?or]¹›L	?tÿ!•r^¿AGN3FGL J1648.3-4611@u6òä¼®¿é©Ùà(ÀÀ7ü¼b~À9íý©
ªã?ý#íãr֌@½•6Þcx?õ:7>/»"?ïò¦æ‰6u¿ÁIYvz¿ÞSªL^¿í‹9Ëím›PSRPSR?1TÊy3?-´&•
¹Œ?é^xrqPi?Çê'tP#?Ê}sϖ¼×?ÇÂðÕë"?5˅ÄQ"?Sv.xjø*?ä⾫÷À?ÄEbpô›?Ö5Ç`c?Ä'|¶MÉ?•d+­ë¦¦?Œ³Ké ?ãäS«¯?¹&^½Qd	?×¥ôŸk?¸çU¼A†ª?…*õ-0h<?ƒo.¬PÙt?à´Dƒù°l?ēÎHÍÏ+?ÝîOH	&?ÄÛѵÈVú?
Z‹#4Ö?My7¤"a?åL<¿#?Ðý2ÖAÈ?Õf›±]ì?ÐýºÉ?J0$ø%?f ¤lÍ?ç"K "±?¼Mƒ°=?Ñ®ñQˆÖ?¼$Æì?iÆò
?"ùÀî»Á?ä"Èö?´'ç·ø?ÕòH•M¸"?´b8u»Ž¤?""wfMmÅ?ƒbhÇÀü'?á*+œ³Kê?¼žŸ#-?Ý
•
ÏÍï?½4S">ˆPSR3FGL J1648.5-4829@u-••ÀxNß·
CÀ8»
Z[–)À:m‰;}…?ΨÃ:VO@	R|N°@N wm?écØÏ[꯿î,™¥qØÏ¿ÓXå~
eÞ¿ã%ö 'AGNbcu?Ñ£¸ã*¿?ËË;©ú?Œ2¡¶ö+(?áÀæäœ?æ½Y¿MD?́Q=#:Ü?Ò|™–òþÃ?ыS¾¡™v?³2þ ëƒ­?­~úˆ§õ?ä[S`­ÈX?Ñ/›	lv‡?ӣޞ}Ñ^?º*–,g<?µQÒÓø?¡íçD_dñ?ãƒÖlfc??¼ÉÆÌÇ];?ׄ†¨âH?ÂSHéöÏ?"¨eîÖ?"Ôzr
T/?ãíTDƒp@?žëWó(?Õrù×åì?Ï+"E†a?ˆ®ï†Ž?!Ñø"º?äãˬ¹˜?Ïì-tF<¿?ávÓà¬?Ô÷w†?±žŸµ3ö?°Ó°Ñû}?ُê¯Çêv?Óü+gÀa?á«[™¿ëN?º-=bƒ¥?°bñ.œn¸?ž€§®zê;?ؐŒ€½Ö?¹*';É?áÂ[þ;Ñ?¿£]Óçô?Ÿl»kÜ?{›9{ Þ?ۃÃBà?¿ª8Æ®MIXED3FGL J1649.4+5238@T}òÿf@CÃÙ?¡ÖÀ9'm;l¾À;ÙuxR!5?ïdí·ËUK@@¸Í'n@À@Že‰¿Õiïk¿áp&ÛèÛ¿å©
O…
¿ç½LþµyAGNbll?ïÒl[?c:?vlŠÐz˜?qx'‹æ?sþû‡e?UEnº<æ?Vž*7`
b?îJ<Ø´½?©	vŽa3?Ÿý»Ip ?£-óG#Å?–º©—e"I?œ·]•U"æ?î7¬GNÒ?"9}þ?›Ëäšsß ?‡§ŸXÚ¾?%àâ¦?€'KÇ?ëÑàR?§?$ãL0©?µÑ²º9è¨?›8þ|±Ò,?§>™1®'"?¢™wÝGžn?ïïúÉgñ?^ga—`?Y.ô<Ê®?YÙ¬ÔëÇg?AŒ'>SÓ?@ĸlŒ?ïeÇ_zŽç?"ô›li?‡¶L'0Ã?Rd¤~×?~èãÄa£?'&U©Ó—"?ïQ<Zá?"ZŒÅ"Â?Œm·¦ÂC?AzuqY$?~‡èOâó?mãˆB\°€?îÍ€ôä?Š*Áð[å\?äî¾w?|	óèÐ{?€ò¯Ý˜??²¾»µuàAGN3FGL J1650.2-5044@u.ŸðË°À«ÎÀAùõÀ7©ZÎyÀ:©6»}ïð?ÓÐӆi)ÿ@Ÿ,¾O¢@]'ßæÚë¿ä÷*JY¿æMc¡ÅÍ¿âÎÖ£vx¿ãZ/ðCۈAGNbcu?ï®z@&Ðh?"Æ-£µ¨?p³ÖÕý?zyÃ>ôQŠ?xA,
?{NaÚáó†?í¨$á$·^?º×ØÄ|Ç&?…$Ÿ'DF?ŠÔ¼Y­³?°Ekÿ¨?¸ÆãY%?êM‰ct!C?±žtx7?«$ۈz®	? ì(œQ:ø?À£'ȝq?«ù€AÖP?îD
f¾Ùx?™oÛ9‰ÿí?M@ÄÆ
Y?PJêôÒè¬?«JV…/ź?™JÔÍgËm?ïëTáÃ?i­¨?j÷?X O`þW?gÖKö¸Ø?PµîÁ³?Oj´;Þp?ïB¡‰ÁÏ?¡£ƒìøÖ?qŠŒÌ±½à?vÍo|=&ø?"I+'ááµ?m‹w+«a?퀽8@tv?¢K/Ô.? BJ)#LÒ?–õ/,îi?§±âUi Ò?™Äá4҉i?ïy5§gô—?z­ÜF½S³?A‹?©¢?8Þ5ö.?Q&µ··†?zd½4Œ£AGN3FGL J1650.8+0830@:œò?Mé@>¢	Às"7À9lž#lÓÀ;nâO?ä~Oz!ëH@¢€Èè<@FÀ—ŠK¿åø~¡+H¿é§ÅËô<¿äIFɤ4Ž¿ïÿi¢¹†AGNfsrq?ïõÜÖZ?<?LJi—ˆœ@?Dš˜ÛæÞ?@ýW詾ß?Còä}?Aà³¾'ùp?í ³Ýθñ?ªà¨¥cc?¬eËi´?¡:šªWæ?¡Ž÷òîÑ?££êû(?îôq&*Y?Š¡r"l?"ýç¿V?ƒhY.J?Œ¯©°¥ë0?|֑'ÍQí?é^7E5?®š"
Kxó?»\>fºk™?¥þ² l?Æ?¹¯Wà«jÁ?¥(ìô·?ïùß¼,…^?>zöˆyÑa?=؎o^?5$w3Däê?3)Ž"p=?.®€Ò­å¯?îÐ~ûˆ¡û?•ÑÈQkl?—Žaäzn?‹ùÙ[V?ŒÃ}÷/TŠ?‹*€P*6v?ï^ µéA´?~S¿Ög_?‰ŒG{,?vúó3è\š?~°ŒÄƒÛø?iR@þn£«?íÇîþ>Ό?èR	C<ï?¦¨á[á8{?‡»1)(ÿ?™°]|ô!™?‡ï»WÅ¥AGN3FGL J1651.6+7219@Z³¿µ@AZ–`)5ƒÀ:ÌÄbšÿËÀ<$#wÔLô?Ö.u{N¢G@
êO²¥"?üÍ+4¾y¿ç5Œåj¿ÞR´úw뿳d™ûœÌˆ¿ÙÕ~5©É×AGNbll?ïè4h¬*°?h™âÊÿÿ?Q9©ôå?XŸ2Œ!'s?^^êx‹'?`³å¹òna?$12?…©Êû¯?v
üçÖkB?t»çÒU°ˆ?}«ñaŸ?€'»–$\?îäW/3@Â?õœ'R$?³¡‡ß¢?ˆYƒžŽU?'Áyï@$?'Z^ý-Á?¢ É?'[ ¼ê?aí@]±Â ?hJñÂ,ç;?†àGVjj¹?€Jܲqüx?ïé¢fOrâ?£§ñ1?1±;U‹õ>?4xòx–?d'r'wí¹?¥¼_
Îí?ïÜ+^=?oráí¥Ê?]§B&#«Û?V`gx`—?eXˆla?h¦,²#?ïtQúƹ?€[;$mA}?CG‡cñ?t¢—
ßüÔ?ƒJƋU6?ycÍ(#Ü?ïä•Ør?bÎ:èãŸ?[¨¼hÐÊÅ?Tü¯.äh?[-C3IA1?U°[6ŽZÂAGN3FGL J1653.9+3945@OËôàM/@ClصýÀ6ÃðÈT˜À:(3Auì¿òBªפ—@ø|¨òþ?ûv'¿aª?¿×Ò9M¿ÜU,Ò,C¿ÒϰōÆÛ¿Ó%°)d8 AGNBLL?îá^ŐËó?ª+k7£´?J&=JN?R|šw°Q?¡{hÁS?©Âos?ïÁ<"ùˆ?}ÅM]öD?ls'ãèÖ?n]äûS?q}¨A¾‰?t= àˆà÷?êŽtLƒk?±°­Je#Ò?]Yµ¥?Ž;Gh2¤?ÃÐ]	4Jú?°»Ÿ¿•°?ï[òT¾?K˜›êB>ô~ªä%¾?Y˜|´Ë?"š"¾=?H@`˜F2?ï3 þŠ+Š?¢'>ø·ú?F_S͋Ë?Pu#ï!¤(?˜Øä'õKù?¢^'#â?ïçÉxœÃ?gbgGD´¦?U'ÒŠ»?S¼t´£Y?ZÚ>o_Ã?aÆñ?— h?êì]¥òú?±ž.Pa?'®C·Ê8?õ¿Ûâ·?ÁøÀó—?°6ýZäv?ï¿ùáJn?sL­«È>⛟eím3>ñäc9ðR$?ùéÒÍZý?sL›ÇùÙAGN3FGL J1656.0+2044@DDãõhÍ@A"'@	‹À9¿å¯ò¡sÀ;±b'¬K¿Å·zº9ñ@üZNU"œ@ñaÿÏX˜¿ãi Æxd¿è%/u5)¿á¬@ÒFøý¿å '<9ÁAGNbcu?ïüݞN?6ÓÒÔ\´?óêʑôh?:'±yK?:*/+'?5 G™o¿?鹿çŠ×ú?"÷娇?qø^H§8?mÛùÁô•â?{G.	ú?€›ÿ†Ò§`?ïE>é}e?m&»ï6?}šŽ›=¥~?qzºÛÜ~?ìèêóP?z¿;rO†Y?ï~ÀüŽ?'<ñʐT?T>Àµ0[º?JiÌ©ùŒ?÷·óQô?Ñ:ø}ðf?ïþ¡"'0?3Ü\è—ú?	Mg³AÙ¨?éï¯Æû†?&Ãaf›¡?Q±ˆÕZ¼?ïÝò;=»?k¾en­Q?[Žóðör?U';}ðËÏ?dFKYhÓ³?eì£wò^?ï±À
#'?mÄUq÷ó?n™íÜLÖ¢?ehÅ.ÿb?wÒùóZ¯ì?aíÎ=§ä?ïè€LõÖ?X‡±¬ŒBÊ?>ð^ˆªãÙ?-W†`…€ë?c¡§ãX
?WÇBËáÓAGN3FGL J1656.2-3303@uépÀ&Ì@`™?׆dÀ8Rys‡À:æ#wÔLô?sÒ­@³ožss@9·?œÎ¿çšç{¾¿éõÉß÷;¿ìŠ?£GÜý¿ïÿˆs¬uAGNfsrq?ïg>ÿV?£¿š$Òôä?]Ê;UG+?^}5Åêœu?'L¡½?£¦!=Aè?ìÄ0«nù?¸cõ+'_Q?"Ç1"‡?–j[¾?´ì®A*ôt?µKrÆcT£?èö"$'?­j£ÿ!~m?´B?í55? û–L¨½3?ÂÙ÷‹Dö?©}*èªÜŠ?ꅕ³'œ?¯©lÙÌ?«ƒ«Ï.Ú?£êQÍ: †?¾Ü[¶?«9¢ýú?ëÂåy'Dy?ÑU
Š?w•M]¨æ?š‡Ö8?À7¿°•Å¶?у™¹?³yÈ!?¬©'µ&?…úö£,aÕ?Š‡l[Íû?¡h'#ãè{?§2öîчÜ?êó[Ž¾k­?ªÔ³mwŸ?­7à±¥å?šÐÌãR]6?¹É31¨!?¦-¡—ÍŽ?î.'j6'?"R]}±?"šA°²E?(ˆX€T?¢Ñ¦~VÒ?'éߛö/AGN3FGL J1656.8-2010?ñŒlà@,%8@¹-´À97
ðôÊBÀ;/[àÑf?ô²Ãú@Mx@òûûcŽ?ÿ`%ßãí?ïÿ›BÞnW¿Û9'lIF¿àÿ£¿é׫»¸°êAGNbcu?Õ¡¬k6Š?Ëô'!ǔÃ?ãŸv¸?Íioqõ2>?¨û;"—R7?´ãé˕}?×jâùe˜?ÉÓJ!X·Ÿ?Û4‡°|ÎÌ?Æ:ëMìG?ÊÁ,›—7?ÄmKûߒ€?à'±ÿÓ?À{
0T?ÙYr@Óôx?¾ò;=»è?º]Jo /‡?£en`.3²?ÒS\ê0?²»pؒû0?܈(P‰¸Ú?»å øÀh?Ñ${˜Z\ö?¶¾Í=õ~Ô?ã:'+ÜÛ?Îû6ÙÛÔ?ØSñ¯/X?ÎÕ¶·*y?"p¤ÄH(?Ÿëå#­D¡?ÞN5úÛm?ÈöúŸæ1D?×Z Šy–?ÂÏ=ø×u?Ä®R÷|Vp?À€Þ?nˆ?痣،É}?³Uèx{œ?ÊKà'ƒS:?°ý|¹C÷?­V@2ÝéN?˜:ò¦BwÞ?Þ-»,Å?¯À±ï"x€?ØûGøà/?²zœLì¼?Áøq´Uæ?¨1;]åh™MIXED3FGL J1656.9+6008@VbøÌN"@Bµ²€l"À9Û²~líÀ<ÇC ¿Ð÷Q¼qq@'¹E†qõ@ûkŸ¶>@¿å eJT…¿è"²ÉF¿ç©ó_n᛿àßZYAGNfsrq?ïø˜°Ä?QC‰+]1ü?2BK¼?0MSB5¤?F|vâEq?OT´ÒiC?ï‰Â0À?,ЏòHT?zfáA>/Ü?&؏Em?€\ÜHóë?… j²ë#?ïQÉ_/?€FÓ¿|¥?}bÒ/$]?j®®[ùø?¤"=qø?zÆÇÑ«ì?ïk)£ß»?Š*"F£?lã¢j»B0?g †I»ú?ü®{xÓC?ˆ/˜žòÊ?ïüD1ÏN?A{à{7Ÿ?$R«R?ãâ‰hÇ.?3µrsçŸC?@p+e:±?ïÛ}öêœZ?h#!˵S<?_Þ¢Z?X[v'î?d'·ÇfåG?b+9''sK?ﲃeOºþ?jçø[u¹l?oLU¥mG4?[Š T	FÅ?w"œI%?fw±	?ï븏 hã?a\x֝\z?D¬3ˆ¾?5äNO
ÐÇ?^8ÇÈZ:?`àm_Ÿ8AGN3FGL J1657.7+4807@R–»À5Ö@C>'ŸÐ€À8¥Þzt:dÀ;³r–'–?×Ü$÷ŽÊç@\z–9ý@ÍÖ©˜¿ä…ˆõ lÌ¿çEȊ"(¿æâ°ä0c¿âcóü«P•AGNfsrq?ïýA¬­P?)
³˚g?—·w·P?±y§Šû?-™Zoè9H?$à;îO?ï¸íßìå?ƒúWÀÍb?mVùë¥À?l9"Ñà?tÞjës½?wè½*ܺ8?ï`"¸¼Ó
?z½Ã‹­¸(?z{‹žO¨?e
ª}¹‰?Š¹Îœ?ua·l±1?ïá¸X1Ö?r8þÀX?5æ¾&Žr?7¾)̂?k܊í¨â?ru‰âÊ?ïþí¸Íý?IÅ͆?‹Éšæ¾?
*ÄÐÇ#?'ýÉ'"?Å"u8¦?ïâ;LÃcS?hF4t?XÌ)¿7'%?Såmkáû?a^ž7åQÚ?bËÂQK?ï¬öRN¤?k.ø꣩"?q"1ü?`\zð˜¹?xڐ>i,?bôU÷ª-?ïûJµ›¶?KÈÿ|òx?Õ
È9&#?ܛÀÐs??9àŠÏù?J¼m€8É]AGN3FGL J1658.3+6149@VåT¿àU@@Bwìàh‹À:•€,
JÀ< œé°2b¿èl?Dþ%¤@¢A]îH@:»?†¨¦¿ê"Õ0.Ø¿ÜðÙ",¿ÛK€:;Õ¿Ö:µ-+AGNbll?ïî(Éðý?`V¤Þ»q?V0|ÑÂÂ?[¾4âŒÓ?JüÍß߯?De9«HsÜ?k?'Ô@‰?{."®"Ó?"à©b4^Ÿ?€ÇëúU[?‡ZõóKa‰?îònu18?ˆëC( g|?Ž(ŠbÄñ6?"«H‡rˆ?'ì+æ!'?vÙ²€L—?ï#gkҕ?"ƒô+Œ|?U´FFZ¨?V
¯4]?Š[[u'?~LHõfšÑ?ïúŒþ֊;?;8¦S?1öYwòš?2#×Tl4?9¡øqðû?-–ÕxqëË?ïÞVÂj¯?jÁ€èH?^ë¤)ÀÕ?\̈FyÑ?bƒ×^¢×ï?bX£Äd?ï|Ó݄¢^?r&öcôò?}šE®èb¹?l18"ƒ}?ýåÇA#?c8µ­'=>?ïîºQu?Uþ2¶c¼V?5úQAi?+'œM:´Ê?^UöÐV,?T…çbà­AGN3FGL J1658.4-5323@tíÏàGÓÔÀcð@uÀ8ž•Ï	½ïÀ:ðàŸèh4?þ-µÛC³@
¶tñ™‹?þó`Åg¨±¿à_Âáø"7¿á¥v»¿êù"iiü¿îÂi'¶ºMPSRPSR?`î^ørêÇ?b^hëü¾?íϪŐîO?²J1¯(
Ü?°û6ݘ¿-?²–F~ü?dëeQ.?¡^x˾?ê=AmÍR?¾né¦Ù?Ç7]d_%*?½«,­ÌÆ1?´_i¬ÈÊ?¡M÷qË{<?ç}òé/ó§?³†Ä-p?ÇØ¥¤{@?° ¯xt
?nWmòn>?¦™W5Ž0?ëéû|ž?©Ä
}ÅgN?½\.\½N?§Ì‰¤ç¨?S3±`T
?ZvEHŠæ?î
 Y¼´Ò?±±/ÜhV?®"\ÛݒÁ?°Ú—Rcòe?u×ÙWäY?{?ŸHùLÁ?ê@Î[ŠÀ?¶ËfìÚD–?ÆN»TC=?¶Ÿ¦æ€Ÿo?ÞÜ,CÞZ?ªnâÈÍéÌ?æ"Ñï?±è("&ÿ?ÁVЏW©é?¦´–E‹?¡æÌð?‰'ã?ëqøáá:?£ZŸ\÷½?»è<6^ƒ:? Cà+SŠPSR3FGL J1659.4+2631@Gŝ¿™£@A¢¼ßï¿@À:Lyãñ¬€À;¾†ß'±÷?×ýißäùâ@ΔY=ÞÞ@­–@ž«§¿çeXøŸ¿äKÛyý‹Ë¿é³_
|…¸¿ØÙ,¸V~AGNfsrq?ïÚ³ÖÂÖ?rõŽç«Ìª?WÊ÷Ïø­Ô?[5&}m>?if­NNaù?plԕ÷)>?ïyB?PÞü?"p'L8áË?jÚD?…_ž×˜™?'):À'd?ŒPitÄÀ<?în=BUºó?';E'´¼Ã?"ì®z¸i$?áç»/Œ?žK©:8Œ?‰:_V?íޕ-	‰¨?¡×@}¥pˆ?•þ†Óû1"?"î¹EVWm?§iÅi̺?›*S]¨Û?ïôìÞ\Ž™?T«ƒêñQ?=Dt/DÀ?=,Z™ÿ;F?MªM$öä?Q@"#qÌÜ?ïΨ<¿3?{q•ë£ue?g'°Kصª?n*ò;®R?iÅj—™?qFzˆ"T?ï^	4 õ?|v,my?'&‹bõ?p5jv–?†W'é"ç§?sFÙb´ï?ï"Ò6æhw?z-òœµÆ?wDmŒ…<ö?oôæq»"?~ÒwF‡³?q'Kƒ
÷rAGN3FGL J1659.7-3132@vØ¿p@¾$çùÀ9;\WìÀ:úszK ?ØY¬Þ^´@
<În7–@7ˆàcØm¿ãV<=%­í¿éÙÿÒL'S¿Ôš©ùQÿÁ¿ëR@¶˜GAGNbcu?Ց
þ¥{¿?ÊÃô÷cNY?±Ym }Ÿ¤?±ø.¯¨À?ãLÌXÕü?͖ôħS?äoŽè²þ½?ϪÅ
ï4‰?µMҌM't?°n~€Þ?ÑÍmŠá´ª?˼tÎ;ÀS?â;}Ën7?¶ÿ¿œXRâ?¿ š¡£Ë™?¤ò¥UbÔ?ÓÀÝÁÍÑk?µú‰ 1¡(?á‰U­lÆc?¾PÃÅo¿?«o¢7=}?£w¤qü×?ي°¤‹?¾Ý9¬t?âiJÙì?Ìü
èf[T?£M;àJË? >:êŠîs?ØÃÂí¥àO?ÍDØ`åÚ?ëÖÖÕ©?Áwôĕú?¥PÅ™?¥Ø3Fú'?¹2½ ð+?º¦/UÔ¦?é'öZmgj?­ßX0;Þ³?²ý§ž±l?œ=–î¬a?ÀuRÈ#ð ?§À—Èÿ¥Í?çÀIeh~]?²FP<?°•µfš6ú?™b"ÆÓ¿?ȳÿ¸ÿ²Ë?®ê"7š'ŠMIXED3FGL J1700.1+6829@X⪀J@Aš¸GÀ7õKÏknÀ;2ƒ
?ñs¯g6@šÿ¬óéq@/EnÛ*¿ãúpø]¢¿åÓFœz'A¿æ`¢›æ¿ê2.™AGNfsrq?ïõ+äñlû?OrøÄà{6?OÖ_à|•!?KAGaƎr?6ôÎa·˜?3Oi±¾–?ï½4òÅ?»$Âû½N?lPôÕK–Â?n5ƒáFºx?s븪-?væH
-Œ?îîbœŠî9?"R©¡ø®j?"ת~ø?Â"©°Xœ?Ž)!?Ë?ƒ®  Ç¨Ñ?ïó¿n¯$	?f:†'­ç?#ØÍÓdÅ?8‰¡÷Ã?V	W¸:Ô?eÁÆ¢{ìf?ïú,ýl°`?;Ý/ëØ"?Aÿ"W*¾?7¹.Yä‰?%3¢}›œ¶?$¥<MŠ•?ï䖑–.Å?eN¥¬+Õa?WæŠRÑù?T`¹î>²¦?^ìÍÅ"´?]nJÃ4€?ïO|{ÀY'?ˆÌãʟˆâ?Š‰Ò½Ê(?"êí¹òø?—U'©?xz"G,¨Â?ïýñÛ#I?@7×õ"Ž9?"A=nà? ‡}ˆÞ`?)JïÒ:¸?>XØ*×á7AGN3FGL J1701.2-3006@v{ 1ί@=ñÀL5äÀ8™'è|U¼À;§ú…l¼?üê·
ÈÀy@ÉþºÛˆ§?øDÓò0±¿Ô'\лnÖ¿àÕë/³L¿åÁáìï'¿éœ!3OTHERglc?¦Ñ³ÙÆ?¦i8³è´¼?çÆ;žÅ0)?˕^®XÛ?Ë2¤Âízí?ÊîP¯^Á›?µeÙIÜÉ?¾QÅçͦ‰?ç9ÇÄF¹?Åxý(Œ"?É0,<7Øx?Áª²ë"¶?ÎæŸ?åŒü?µêR¿·Þ?â¼9ÄÇŧ?ºðЦåÌ<?Æ(y¬û\h?¯Ñg'?·e&"éú?¢Ytzü¡?å"[álû?µëõ6AhR?Íÿýj"5–?²ô§J*r?»Ž#óéàô?¼'ǁ&?ç¶!~nµ?Ë;aMçƒ?Åæ€T´?Ƶֹé"÷?ʤa7—5?ÆÓB"œ|?ãÇ֙\æi?ÇÑöU9öÏ?ÆÎ9TÏ)?À"ïèO?Õû <ÿmg?µOcü!û³?à/ˆ^2æ1?¶U€lÐL"?ÃJž
5Œn?«§ÏW	´Ü?ÃÂ|¥½=?¤y€wô(<?æ`…¶Z<?¬KD•éÞA?»lQ':?£vaMUPSR3FGL J1702.6+3116@J³Ÿÿå(
@Aá.ßç[ÄÀ:T'Íó=zÀ;Øèd?ð¼48Á½z@Ó/ Tk?öV‡¡ž&¿ëRHíã%‡?ïøvP`·ó?¿ØSË{‹^?·%ÂåËÔÞAGNbll?í[›¬:Ó]?¿w‡Wïøm?'´â›!KX?œ<-Ø«?°µé÷ÏÁ?¼Gad/:¼?ï":'¼?†'Ëþ™ï?xú.ùø\þ?z÷r¦ZY'?|ø3÷_Í?€M^g?ê+ÔÞØØ?²Áâ.8©?±™^/ ? ˆõ5
s­?¾+ü´Ø ?®bîµ»õ?îî'ÃO†·?¡ýä½q?‹ÜÁŒ|Ћ?™¯MgÏ?"AFÎòØ?–Q'.W?íU¥>úwç?¿¡	¥p<~?1–ûځk?—®ï¯4gd?±FpI£"í?½¸AFé•Ó?ïמ箜Ø?sP'´ö©?`Ò¯¾2Ðï?[¾ÿüš[?gŽh×è†R?nt=k§¸%?ìҍrç ?£ÓÒÒ)Àß?¦«߯´?–Ç]µz?¬3GI"…Q?÷Ór<?sqøÒ?ŠÊl7p5›?ƒšëI§£?ˆò-'1â?sö["³Ý?r9ŠÏœIAGN3FGL J1703.6-6211@t'%¶™…À(Ü>úç'À7ðª4À;?úVôÙ?ìÔ:>a±î@…g;Mˆõ@È£Ìhú¿åE:‡:qk¿æU/ø¾¿å²Ê]ZÚ¿ìÒºû15AGNfsrq?ïì«ìÏÃï?\¦¢Nȇ½?W|o@Åb?Va6µ‰q?NWm"øÞð?H³ûi8?ïX­«å<?•ˆhôÕ^?s©>¯™î?uàýªfû ?ÿõáF–?'…¥{7s?íš
ª/
|?Ÿ¨"J7?¤vI£-t?•-p°Õ?¡èÛ·{uÐ?"5êEú"U?ïžlEàÏ?‰ޏu†ó?T~3ÚöwÀ?_n'¨¨?…Õ3qÉ%`?ˆá:¢%?ïïVzø?_ùµÜû?WCjX?XœÂďTZ?D!_³Ög<?D
¶ó!.Ä?ïÃÂ!¢‹?yJsû'
?`C6áš8?].¦S·È9?uýT³±Z?tC^ Š¼?îIv–ŠE"?——GՍ­Ö?œ}-à	Ç?Œ¢ZÍèx?šSÿ‹¯ÙÉ?'""xhÒ?ïí›v¾xK?c³«qêõH?@E•a"aæ?N)Yžž$?\¦Goݵâ?aæð:–NAGN3FGL J1704.0+7646@[;ɟâÚ@@3S 8"¬À:gCÛ÷ãÀ<´SYCh¿ÙúhöRq@"cW=@—$ žE¦¿æedÿð ö¿çaÕN•S(¿æõ47?1n¿ïþëWýBAGNbcu?ïýþ&GM®?%ªøÞµ&?ÀûïÆd§?$ùEmÔ?$=ž"HÚ?|Ñ÷ˆ²?ûtˆœ?‡<¶ç¶?vŽvþyé?s9¼pPx}?¬Œb?ƒma_DùÏ?ï\;g+«?}{°¢{?‡¥…RhA?v(‡œå©?å‹'tQ+?l؝¨ÙeÕ?ï³Xd›
2?{õòzÑ@q?c™àÉQjÈ?bïiA{"?|†Ýl¾­m?xo¸‡3þ?ïþå0Ï^U? ,õ1œÄG?Pk®{–?Q²ýµ2?ïŽîf?•;¨?ïÞTI-p|?h›þbÃÜö?^#>)KŸÜ?Uƒ"Î"ð•?bšÿâ4#?bÍ÷äbt?ï}O2\Š?sW¯'!Íl?"@ã=³/?o‰11ÈDh?xÖ ;Æhþ?`Ùɒ_-'?ïô|¢¥%?TÒþéÌ?8)sÈ´~Ò?1>5ð¨?Pü^tz\Z?SŽTýjqáAGN3FGL J1705.5+7134@Y¿B¿˜0ä@@õ®Ú«³À:¶ïº€À< VrÓ\3¿÷ýò ï8Ý@ùÛQÊÍï@'¿_Ñ̼¿ç[¸b‡‰¢¿éeÈ­´¿¶x,rµæ=¿ïÿ"m¾RAGNbll?ï¾®ñ'õƒ?ˆ…:l³?rwÿ+õ?ƒùü]A¥@?lar»
?oqxøî?陵4Íp? ÁeGyދ?"GWÿܟ?'=ʪ¢oE?ŒBR^<cm?"¹•´?ëä>©!?¨¨a¼D¤?²¥ÊILÀœ?¤"»×€0Ç?¬p€Û,˜?—Çg-Öµ?ï=?†ý?"€¢
Ð?f˜d³!>?v›o²í_?•…rv(?"º,¬É?ïã›/hDÚ?jêtGævª?YËÁ•­?aÓ6t?^þš6æÞ©?`àJCu>©?ïÁp×>ÑÞ?€C"ª@P=?oÛƏ=+?sÀ|ElŽþ?n³e Üå?rV˜ÀéÝ?í"(oϋ?Ÿ
]ªÚ4?©M¥÷·6W?›©SÄúЩ?›.ÿ(?†Ý‰|xÉ?ïâêë)?c¯r"2)°?=—¼7>;??)ц*1?icû⸔?b=ú"ÂÃAGN3FGL J1709.6+4318@QŸÞW9@BƒÀ€æÀ7ÇÎÄô'7À;7[‹AB?ö(ƒFÆãÕ@b!LÖÈ@Z"tf"¿àóÛõ3É0¿ä³"›Çµû¿äÛÖS‰?¿éU*m¬AGNfsrq?ïô"eìݨ?Mr•
§!¢?Kãë­þ¢}?HTdVPF?AÊ|'rƒN?7ÏÅɶœ?ï¹jcmÊ?‡¹79j>i?oð*b
Ã
?']÷ѹ×?sR饁IŽ?v"7.¾M?ï†"í?'æ 'ãV?ŽÀféÂF¤?‡`['»¦?Š{÷ûNE?ƒý^°§Œ¨?ïùeZ4?UT÷#5?	aO·z²|?*í}ÇÑ:"?HՑ#lü"?TßYrœÞ?ïùfHçØõ?A
øZ²ç"?B¶Õ^ê/?=Q¯˜?.ÀŠ'?&ñvâ
V?ïç¥åK?en²Ù
OW?T³{ƒŒ›?RQJQ<?]µgt5?^™ŸÀN‹?ïm­G¡ï?…"Œ­8®?"ž\^<,?}keìå?€" Ų¦*?yá|hMŸ°?ïÿ#-£ô‰?2߁ílàÂ>ë0&‹ÛI>û=P[fîÐ?4D°åëË?2²ßÌ^)-AGN3FGL J1709.7-4429@uq"_ôöÀƒu€_¶ÊÀ4s 	ŠÃ=À9Œ";±†ö@
Êϓ%·@îô¿ÚöÜ?ô…¼/E½Ï¿Ñ3JøLt¿ß[o˜ÐW,¿äDb"4o¿ëž©<·ÁPSRPSR?3ÃÔ
'a?6Ǐ}îŠ?åq<BGð|?Ïm5¸s¤g?Õ¿‰Ã7Î?Ïm4$¹Œ˜?3VÍ®Ž?q§K¦Ï?ëºù'k W?ÁÑw›0â?Á
oý`_ß?Àò~ˆØ<~?':ß°Bh0?'ˆ¾nÝ#?çœÿïÜ=Ð?·	§d‰Z?Ð4)# &Í?¶ÕÐEÙý-? CëØþs?2ïÇM}È?íc]2"®§?±Ðôãaü¯?´ÜôvlÀ^?±Î¯ý%ˆ?:Áóhþ?ï6Zð?è"Ý]úÃ;?ÍëoqŸL?Í­£.÷Aô?ÍêÅó·Ê?RE-²Cø?"w`­?ë-?˔?Á*`yšÿ(?ÃӞÁ)^&?ÁT³$sì?jù¨_ö"?'¿-ђH?æ_ËılÁ?µ­a¿¼?ÒE©#-	?µö9+?ey"(W?^zÒEL—?ìˆÊ_ÆJc?¯jA{ñ?»±Ó¢)
:?¯/¯PPSR3FGL J1711.5-5029@u&¸!ïÀã
é`À9W4Ïëe>À:ûy€žQ¿ì~Ì¿%@÷þ;¯®"@võ_"
Ž¿å2­[O¿¿í"š¿\æ¿å$˜ÎmG¿¾•`åHÈAGNbcu?酑ü[£?ÆIw/ï@?aÅr#'´9?\"U~×âX?É¢¢E©qB?ÆC¿PÔ?í¾Â¶¦ù1?ºE"»'Ä—?†NèÇ£=?'EسR*Ú?®€"R?·"ô_I!î?èµ1Çð'o?´‹Ð`p§4?§:ïn}Ô?•ºêµ©å?Ç\}+!
?²›{¡*x?î*ÖêvŞ?ži¯˜°ý?)ó^ª•÷?1øˆMä?­8ùw;%?žck&½Ð?ìooN—h?ÂÃ."f›?R @Gï?MÍÌø‡õ?¿T"¼4F?¾Û/ïx?ï^î9¦aK?›S(I‰Ü™?nCÍP%•d?sˆ¿…Õ*3?Y¿'â`ø?—-«™¹?í+ZòòÀ?¢ýË^—øË?"fC)@-Q?ˆFÀ~–Ñ?±‹Ÿ^«?¡"k¦|?ïŠÅ"ßS?x­¹Ë?ëゥ
?{óYwöE?$ßZ†¼?x§12))cAGN3FGL J1711.6+8846@^kYáó¥@;£Ó £ävÀ:p*ÜLœ'À;Ï(†1?âSb;+ª@
>àI+m?ù€@'&5¿î
rÓ©'?ÚtDìÍ¿ªmvûßßÏ¿ÇöÀÍK^	AGNbcu?ïôê*ß/Y?LžÒFM™±?>øuîL?6kBH\N?MSÙP-'©?F½c¦R?ïˆMP½>?&ñdz&k?yán"þø?ƒˆ!1¶?€ûôÀwM?‡'Z6â})?ïU\ 6c?…z º]$?"c+>6?tt$³÷:?"£"Ø\ˆ?9—=Û@ ?ïXé¶<''?âþ>><?vÑÞÞ3â?nÿ3žµZ?Ž\¢õP?‰G÷{Ò'b?ïù¼	Ž§¬?@4#¶<Œ?/‰…œhÓ?)÷§¿?A-x,@u?9ä:_ïs?ï×Í/Yp?sÝځ
j‰?aTŽ†?Wö)-ؾ?g/|›+"?p~'}¾`ê?ï€7Á@[?v‹ŸPRÖÏ?yv"—sË?hf½ˆs?ƒ6Åܒ'?rÁ¯Z«?ïÂùÈáä?r«‹ü¦mã?qˆ"Èè?kÑô'ÓJÂ?jÐߘ9î?cÁ%Ŧ"AGN3FGL J1712.6+2932@Iýöÿ¦=í@@ ƒ?»òÀ:D,_Ú[+À;›Ýj©Â?èàðÑlwU@Öa¤J"?ù4ŸWž¢?Õ-­zË?ï÷NÈKD¿ä¯ÀU"ÏÁ?Écu‡ãÛÿAGNbll?ïÛÈ<¼–@?pⰞIÕØ?a¿•
]»?lSÞ'?bx¼Å¼¹ä?^^ Ç"ÐM?ïTÓî÷fv?¢4VÄl?"°iu× û?•Çë²-H¿?†šÚ
1?˜T÷iˆ£¶?îm4¼¨Åå?'>'ïÁ?—ïi˜ÎW?‰Ã}I«?šjaúo=?†+Ûã܁ø?ì}ñõü?ºÌOAJ?±šl"5úÑ?¹Â"ãÒM?¤ì"b¼Ò?¥p³^v3â?ïóÂ/7?RÀC4Ð[?F&1?¯—¯?Jï´Ò×n?JÑ
ìû2?C$yõ'b?ïÊv-®¹ç?'»oDÂåá?iÇ/Ä[ÁŸ?vwRNHÉ?k¢^/§`?wš¦J\8ž?ï(‰ÙT'õ?ˆ7&"w¥Þ?‹Û6+'ýd?ŽX¨Ï¡?ŠS‰˜YN?|ZwâŽý?ï\š'½ÝF?ŽÚ}å^1?ˆ¼DÒ2‹o?†ô"Èì›ß?€t·;.?}Fì<'^AGN3FGL J1713.5-3945e@uµ`ûH
¿ÞCë c¼'À7m÷¤ç«À9ڟ¹nK7?å…ø¼X¥!@
t×½ìŠ,?ùú¿˜†Ê?Ñ$†<oœñ¿åÅoá9k\¿ÐJ)"]È2¿¿þE?Ð$›OTHERSNR?LØïǂô?"vw~ÝBË?~0ê$ÕZ?ƒ«9ŒŽ"?ïA7d4 Þ?™ûÄt:!?³‡æ,´?¼†¹ìÒã?°ºЖ?®	¨ãHA?ëœwÀ
½?".#1ú?É@
ŽUe/?±
þ.9fc?°
ÿ/Z˜?žôj)ýE?箜¶"ñ?²…^—B¯Ü?ÂÒh!ýU×?»ôÔÖu?{€ZŠiQ?†AžFVÅl?ëeB$Ø?¼ÇœC9ˆ?…D²\…ï?Œ
¨nä?'ñi$^ìŽ?†Ø+7¬¸²?ï_'"upÎ?—«-jÇI*?Èóäžz©ê?Ï-΢î_¢?¶Þù[\X?¬ÅÈr[Mj?æó
ùz¢*?ÐP¡Ù;õ?Í´.-ÃeN?°åKÆê?µ¹¯L?¡ÖaTÃL?åð±nÐÃ?²á2›™à?É!tJeåô?Àþ]¹ø?ŒÔsì(5=?"(í8?ö?éDQ~ëî?Á"Í'bOTHER3FGL J1714.0+0748@<È%ŸÌ¹'@9/(Ÿ[zzÀ9cÇÚõ"|À;hèz0H?ùÐÄÔú@
ÕÑò¦{)?ûڀ׫Íú¿äþ̍¦‹¿ÖêDEÃóN¿àfr†ýr¿îÂÖF¯MPSRPSR?"´_¬ ?¡¨r·mð?î³I/Á0.?¦´uŸá© ?"âÅ­TԜ?–«©³åm?©Ž£û«:?·?B÷¾–h?ëÅ[¯(L$?ĘƗËۃ?µ
ЊŸë=?½`ÉÄY¶«?ÁŠÒEK}q?ªéyÚ BL?èã·áix%?²ÙÂoúÚi?µÌœi¯Px?¢?<ƒxvÝ?ÂÝÙ1 ?°ß,‰(Ë?çßè·L³?»+‡éÕ‹?¼Èþ"£™*?¬Ð#6?œR)y"BQ? øØgŒ`‰?î'1Ôl?¥ÀE°rÃ?'‡›òÂô?'

Yò.?»°b|??ÀG;uCp?隇E·¢Í?Åô¼K?·{´p#m\?·¶³#%?ՙ')‡Û#?´µDw¬ž?âځEºÊA?¶%åˆÁ–I?²Åí)äò?5Ϟ"U?ϗÊ.jæ?¯ê	âk•[?æç¤5÷*?³uÓÁ³"?¯Ò]nÈÃ?˜}ÑÇEiæPSR3FGL J1714.1-2029@	µŸ´Á@%,ê¿üÚ²À9åRÒ4ëšÀ;;h7÷¾?ÙÅ¿'6{'@{6¢0—?õ€ïÿÕÙ¿ïÿñã?ïøËùo˜?Ù8'2"t?¯ÄõµE¾óAGNbcu?îîqÁÓ
r?¦h#DœŸÛ?Y䮿ÀO´?Zµ)çè_? I¾nröÙ?¦<‡þc30?ïRÍzFÃ?U,oY0?s‰]¿×N?wtNŽ\ê?Ãù>šÅi?›ÚuÜð?ì×.¾À€Ê?¤°;wžsÓ?™Ußÿ†<Ø?jý¡lQ?²ñdDö?¡ÛöFo…?ïOd-d?›ÚVŒÏh?KDžšºÞw?]»8F3¾?•D'Îä?›N›Jr	Ë?ïIžb3ÚV?¤úur5?NýÖ».
Ò?_?™tç?•ÔE
LêQ?¤ï‡{£©?ï½ÀÝýn?‰ŽÊ҄nP?_†'KÖT?`*¨só?y>]¡Ü_B?†šÇ·§07?íç@¦ž?¡0|ÅYƒ?"­ŸNÔ?'ù!ˆs©?§%%Å?W.k÷j?ïÉM=m?v³²–—?P¼w"]ù?REa}°DU?w*C¶J–?uŒ<'™&'AGN3FGL J1714.5-3832@uÆìà2Û?³´à
ŸÀ6‡à3±ÞÀ9©Þß)?úžÉ|5Z«@ìNµo¸õ@g(ñ:ë8¿Þ]›ç|¦¿â¥¯¢šÜ¿ã¾¬B鉜¿íÕÇGQÎOTHERsnr?Y4ñ~?S×¼©æÜ)?ސÅóÈAÖ?ÏÙÒ4ÑÕ?à«ú/4?ÏÛ~|W%?a'ë{¸+?vÚeªpÔ?ÛÁc()¥ý?"+öJl?â
»Í?«SY³'?¦`w"N?Ã?šŸñ¯÷þ?áýSׇT·?µtnìæ«?Ù9I_þø?³û~ÔmìG?™¬r40ü?–)GœØ°‰?Ñ7$7…?¸¬'ïyN?æ¯ç
³Å?»L3IÙgæ?j#eÀ¡í?rÚuû"n-?؄ž£wF'?И$!{ˆ?㣍Iâ¦?ФWp²Î'?wTzGói?Š©¼¦'?âkìNê–.?¼žµ€'?ÚÊÕxU??¼‡o5?¶‰¬äëu±?¢¬gºìÛ?ÞkS'›šó?´§ÑM£?ÛòA4—{ ?³È¸cøè?œžîƆ\‡?›æÛyŠpâ?ÑÀÊNÜöª?±ëÕ°q"?æ:£bxΦ?µÿP°­MIXED3FGL J1715.7+6837@Xә`#VF@@äå@a À9˜hô¶âÀ;Û k°R?õeڍ)ɨ@üÓТ?ý­ËOt1€?ÃØÑgç¿åý–Pía¿å(z‹LÇ¿ã
¯ÃžóAGNfsrq?ï÷ä2øƒh?M{Ih¸ˆ?3ŸpYXù?1'j`?FŸ|È:A?HüSG°?ïjWªi˜?'‡½'G?€™‰õT[?ƒÜEx žÈ?"Ñ4O7×¥?Œk50£à?í?YR'Û ?¥!ñ¤?s?¨"òՋgq?›§züÍ%?£…wÿ—?›ó˜{|ò?î"ÉÝ~Î?¡¿ù'$?'íº×Lš?Œ%ã?›™	Ð?žg;{뮛?ïü±w9zÿ?1…qà8ü?.¤õ@t?)•;ûm?&Cû9´[? å=på?ïΰºÈh?u‡®Vmm?gv¢6á¿?`uÜòԜ?jÛØcÇæ4?qy…lƒé\?'ás?—…ÒÓ§%?Ÿ¦%NÊè?"»`´bØ?%'JÕc?…¢™dÃã•?ï›óëÁüÝ?€_¡ïð?,tŸ.™ô?r˜ç©-F›?oZAã¤Ó}?tQÞ ´ŽéAGN3FGL J1716.6-2812@vRÿÚ@S@ä%_µóÀ8ÃÆé]ýÀ:Íõ`iÍ#?ñMD¼rŒ@ÜJ)ÄÊu@ê@¿Ê¿â¬
µe§û¿è&Õ¢}þ¿ãÕíݾŒ˜¿ïÿò"²¢OTHERglc?۝ù·ÞËt?Ëë"'½?Í뻣7Z¾?Çì1×h‡(?Õl(ur¦n?ÉΘim×Ê?Ò°>53­E?Çö?ÖÅ)=·h?ÂHôÆ;
G?֊˜º¡|?ÇS¯‡[m?܆Ÿ=¿Ë?´Œš¦¶—ê?ϔ­¥Ùݛ?±Êlƒ–5?Ó¯	ïSE³?³æM^O
&?Ѝõ2éٚ?®°áã?ÔÌH"Xšv?µËq6ØÎ?ڥª½‹ð?´iväì[ç?ä§þê´È?Ê`fÎ|`Š?ÄuïÂÀ¯?À'Œ]ù}?ËOpô'l1?ÆÃøî
W?ÞeP'½Ø?ÈعŽ›R›?Òp±"Í4|?¼Ö.Ür˜_?ÎáÓBX?ÂNjð8·¬?åG‡®_¤U?³1,
>\?Å)=àz?¨m¿é=?Ÿ£fW?®jü/2j?ÚVŠ®Í¼?®þšÞ¿ÈÀ?ՏtbäŒî?¯-;h"?ÐQ5l¥V?§x
¿ŒMIXED3FGL J1716.7-8112@s{ fèÀ7U* ½zIÀ:—íùm?À;Îú2`¥\À
ü¶!9¶…@
æÞÿ)k^@zñ –¸ê¿êÐ熿î'ß«¡¯?ès›s
"¼¿ç"!šYïAGNbcu?ïè8Íô6–?f ×Hú6g?!m<N÷v?Q¦Þ#Ÿ?f°^{788?f?]¨ÇÛ?õ@¦?{ÜõWé?hØͼë?tÿBêXz?…`WŽkÅ?Š‰_;€³?î@w¯l?"%BXa ?…f5½Fà?pBêAÇ•?¦º~õ/x?"~ÕúN?ïݦ˜toW?'Ž&™PÚG>¦D›Õ75>ÑQGϚ².?q, Éû•?'ŽÂlaS?ïתּ<Yx?abí`>?H'¡\©?­eˆ?^ĆzýT?a2ý*¨5?ïÜv\?nð²:"dw?SUÐxFg?SMM&€ž?iÞ»¤Ú?g€2L)"?ïBS%†?Žœh̊A>?vÎ-\Fd?ZÓ2P—ÿ?˜ë¬V¢³{?Ž‡.´ÅŽ?ïûð|\ûa?D¥+‰Fa>"œÃ¾sEû> 40LÊò?@<Ãü(åé?D£.»g(­AGN3FGL J1717.4-5157@u»`(^ÄÀ (g "I×À8›.­'tâÀ:îs#ä
×?íŸÃ'™þ¢@Í? §?@óNi¿áµh†•ö¿æqÃóà7¿æ6ö°RÄ¿ï1æáPãAGNfsrq?ï!w:ná?—o….Ä?mÅ)ËA¦?l3تV?˜sƒF×?–R´$VÃÓ?î¥oö)‰ß?« ìî,"[?ýîI˃R?"ú²L鞲?¡©BÖ®*?§ç½¡³.ñ?è¬
M­ï?°o–Æì?°ÿ‹:?]š¿þ@	?ÄÐW%«¶'?­žÄÙfͺ?ïC>H±?"4¨"??`ŒÇG?pÇû°Ó°‹?•—T±7cý?'6£Þ.?ïsÉc¿J·?óÞ —?pw˜ozp?möŠ<¯µÇ?‹kLä'
?‹-IpS¨ˆ?ïbËø͗ß?›2&‰OÌ%?oÒà€¿s??r²…Ž,¦?XIµY'^?—ÀȀ¹ƒ,?ëm9/\Ë?« é¦ïè?©YTÍ:Dš?–¿æ¸Åԗ?·éŒXkï?¦ƒ€P
È?ïËù2†e	?qú±\¼íÿ?O—ÇRè&v?IvÛÀ9–?vmµÖ?q:@¬7<íAGN3FGL J1717.6-5802@tÊ*Ÿ{ZêÀ'¦þÜêQÀ9KHÓ®hÀ;_	Ÿ»òŠ?u 5Ø
¥@÷¥LUC(@]€†£¿ä."Š]‰¿ä <Ð.Åտ䅄 |üo¿ïü¸#Œ:ûPSRpsr@?í¿gdpËx?±'dž¯?§ãù§/á?ªL­lZ'?˜K (®8Ò?Ÿ
|J?弲⯦æ?˲ùD­?ÀZ;%×Y?º;qèr7?ȲùOjT?´µ²\'¯?çŤðñ5?±›-{4êó?ÄñD:ífË?«8e"\Øn?·ðP
‰Ä? ~øˆ±L»?å¸WÄb?¶Ë)ð¥€?»<YÉ0FU?±"@!Ö?ˁ¹¼WgN?±·ÀâÐó?îæמüž»?±½nTlIò?™î·‹Ð‹Ò?°.ÕŠ`M?'l©&"Š?"C‰Ò??ë·Oõ-5?½08d-?­aíñ4¶?ª‡8Q¬Ð@?³"‰]Žù?²¿Ff·%?ëôô¤Q?¤o¿"Ôb?µÑ5{Á?ŸÍw!¦[?¥JÉ~?'·gú~ûw?삻›™pv?›÷a
¡•? 5΁Îcà?Œ¯~)Èóœ?³Ï;áoß?šƒ¤]ï~»AGN3FGL J1717.8-3342@v/€Uûµ@ވj1À7,ò³"À:(zúr!†?ðäH™w@ðU+%É@HkÀmmí¿å—Ì<%—Œ¿é3‹fŒ¿å¢`°ì¿ê½]¡¤^AGNbll?åùj•à?ÍÌB´ì—? !Dáù?¦ðV̌Øb?Ó¿êc%A?Í/ä‹Ò¨ü?èëîÛ6êD?Ñ]¤'éH¦?"à%1LZ?šÎÇR³ù?É´?ë°ñ-?Ð1DÀC?áË\4?µÜ¦É'ݲ?Ã捷§æR?­fõ¹rUr?ԝ's°?³U­0#?êÞ-Û)Ý?µÉÞû‹l©?wnÉ4O?xAÎÄ^?ÃËÓw$¾j?µÂ˜%o3?çW¸¥ÅÄ<?Í /(NÊ?¦%l\ZÚþ?±NQ;ìF?ÍÂQÒ8O?Ës€FGž5?í¹Óš`,Õ?¿šª?…Qߑb¢é?'‡¬Ä_9?¯Nu¤‰ò?ÀÃ¥lò®?ⶅYŠy°?µU5Û¨4?ðîÊÎoå?­Ëd"eî?к}薵l?²Ï -)Ö?í»þ—äÒl?ž«ml(ä?tÙ'ÛO,?k…ær\E?°Òxҟ€¬?žRæU)À'AGN3FGL J1718.0-3726@u۔€u?IJ¦ ÷­‡À7¾"Xð\À:I窞¥?Æá-;¼@
Òfhe@+äU¿çß'¶ÿ¿ãáäŒ3 ¿ß"ÂÇæ¿âœúÂSw OTHERsnr?'aßݺtŸ?"\£¦?}@+ÿ¹9l?~Pò-¨Þr?ï:p©,Öð?˜H5Äg`?«Þ­"ß?µyÒj¸³û?·"â÷£¾u?²‡Ãì?ë\õÀЮó?ÀN=ÆÆ4?¸>Æ®:`?¦gáQjh?¶MÃÔSõc?¤
Ž9gÍ?ê.nÅQû˜?°ñì÷ýŒ?ÆìwÖ	þ?½D&µ÷HK?"ÜÂhcÏZ?‡°X伐?é¥û÷ ¢&?¾«¸%Üï–?'x-µ±,?1©b'Ü?'î;Ût?Š­;%ߧ_?ï,CPãf?˜4eûAW?Â0—¦¿
Ü?ÇÿŠžBår?¾uîLVù??±CÛE?ç¥LÅ^!?Ê݊A.jï?ŋ)èzJ?«¿kÕÚö-?¾+pE"¼?¦Œ"2é?æ×Ñ÷ó°Ö?±tJ'¬®y?΀/˸?Â:JM;?–Q¤VnÉ"?€	j&'R?ç­gÂÿ?"æp0OTHER3FGL J1718.1-3056@v0÷Ÿ©~@ !€ƒHÀ8É&رÝ]À:»_"K|?ä™fîC@ÂN™–@þŸßXë¿Ûi;9ßA;¿ëV¹"uÝ¿å#m\=²¿áTn‰ËpVAGNbcu?ېp¦bÀ?Ìõ ¿Í?Ÿ×<q¬?¡lÖÍç?á9
ÈôÏ?Î"O^»×?çöH˜ín¥?Ñ
4ë]öD?¦"mÉF^?®<NT•¼<?ʅÂ4 ú?ÌÙ÷(cÕ?áNL ö?¸ºpVcÀÃ?ÀÏF
­Ä?©oi¨ ?ÔüÐ`ç2?µKdèëo?Ù¬W¾Ð,J?¸î¨'D?¬¶A7[K?¥5s
šÕ?áhx¼vµ¶?¹Wüiº"?åw)ãåSh?͟·7[®I?€úü/Ø?ƒCÍÞ½^Ÿ?ԅ¤fž'ó?͐ƒ£ìŒc?ìý©õ˜",?Â}B‰E=?™fX~»)´?§>ãAb³Å?±¹2C9µ?º"¸SC?é»ߚs£?¬fÐËÆ?°'2ú>¥ ?œ'£+?~-?Àʛ÷³"?¦§ËV!—?ãù;;H?³)áï¬r?ª§Õê®å?":–­?¹Š?Ô¸öç'–ó?²%«8O<MIXED3FGL J1718.1-3825@uÏÀ7"¿Ûe}`††À78CæߝŠÀ9¿6n@O@!w¤QX@î!è2-û?ÿ£NÏ?æl>;ÇMÔ¿âKW€–¿æ»\s¸"`¿ïIV^0ÎPSRPSR?SÓI^²Ù­?RsUM5?τÒUUzŽ?ʤö[³ÒL?èáÅÇ
à?Ê®ž#/—?AÊÞO{Ò?VÆ8'Ÿ'Å?âF‹Ö(?Ä
ªk+¥©?ÛjäG#?Ä—áwm?"#þé¨ÆJ?Šq'šy?àj×Px,P?¿Rÿp&óN?Ýøpãz?¾Ë[*é?ƒm$áUÙÈ?€ÜîÌíü?ÞØgè³?Â`¨íZÈ?àFx0'?Â]¡™ Ù?Q")0÷?RîÙ&e,?љ.\+Fw?Î}&º\W?ç*èÞ<?΅ÚNYn?RÌDZä?lr3§?å–Üœ½TN?» ¸0À?Ô¿yÿÀE?»º½c?•nÞHäå?'E\[ë?á8;¨Ñ?¸f–ÏéH?ۈ¡¤ªï­?¸†×¯Éå?‡8QÿFߝ?"ä34¤'3?ޚ¸_yڄ?¹">‹·öÕ?àUˆat?¹äƒsx®ÏMIXED3FGL J1719.2+1744@CÂIàâi@<A_EàµÀ8Ãp@Ú»£À;L':ƒŽ¿è*"öØ[@³>\;-@WhÿóÀ­¿à;Ý
·£›¿à%–¯Yl¿àÿ[Ikž¿ÛÆ;IheAGNbll?ïþÐCé}¡?/Þ+mÒ?O^J>ûÂnV³É3?Oÿ5d¼ì?¨×B8YÒ?ï¼£Ip·M?	á"%ڏ?kð7ó"Ø5?nI|»‡i?s¶?NíK?zÞ,ýN?|"v‰?yVA¬zùB?x	«Ý	w?mLAçþœ?ƒ["03?r¨íŸ(B?ïûlˆÌÃ?IŽ'Ã>»Ü])9:>Í'+²Ã¬?BA ¼¢M5?IˆYÝç~ƒ?ïÿF¡úç?ÑgW½.{?H"êÆn>ö­YBãw?
tw•ŽÇ?‰à}áЖ?ïåÄ!"µ?izFÇô?VR…_n.?R…ƒMÙýå?_peJ¶øD?d"ÚD·n‡?ï¸tÄøî?iê7öú8d?o•üv²?`ÎN	˜ó?t}ú¿"Ï?a=i'Ò?ïÿO@…Z?{
ëáRn>¦WÔæÔ	X>³%ËtCé?ëB{Md?hà{
¾ÂAGN3FGL J1719.3+1206@@ÜLŸëÃ2@9Ö4 ˜ü¼À9ð5³@3ÍÀ;~#yÌ?ÞüRF…@Q8!.£×@ŸŸ÷ג¿×r¯'¨ï¿åêà`ÓT{¿ÑŸ!='\¹¿Ø]0Ú_ÔÉAGNbcu?ïÊJà_7?v³¦¥ÅD?Yò¤p¯p?W}ÃÂ
‰\?t]æí4ÎJ?sÿYJtÇk?îþÈ?t_"?¥F¾é$ë?Œã:dR—?'š-§7z?'µZæª\? `_m!6I?îYÄÎ6ë`?"xÐìw-?'f›õ§R
? §'¿.£?¡°e#unû?'
´,ûˆ?ꉤ'oS ?­ß¦¾!6§?š ER'?œwbòoqó?…eaem?©…ãÜÃ@Û?ïé,V5[?gZ³4â>0?IG''-ß?Nr'l®Ú{?`'ó§ˆ?bf^߁€Ù?ï¹®ÁL?"âýžxfô?p¶<:4ƒ'?s¡vÀè?r¼ìÎ(¦??Q
á*þ?ïUOdŽ—T?~Íõ¤Až?€Àßâˆà·?r~ï°{*?‰ëFìjÐB?w'¿BE(å?î4ßÓÿ?'÷«@⨔?"žØÒýY?";â¼a?¢â¢j+J?‹¸€EâAGN3FGL J1722.7+6104@VŠÆŸ÷¬@AàP7PÀ9ó¡gÄ4xÀ;ŸáÝÖ
?ߑ±ÿÓ«@{7*ŽŸ@øýŸÓo~¿è‹t­¸¿êTÓSFŽ¿ë¤3Š\]¿ïþ™øRü@AGNfsrq?ïæ(M0ñ?cÉ՗8г?_"í¨†'À?\ç'&֙'?TõO$í?QÐ~,F?í½6³à?¬µ~çža?¤—{üŸr?¢ç-¨ÞÌ?Ÿ/*•ˆq?¢ÀN&c?î¥û'å2…?e
|Íß[?—¼ù±a€[?†tnGß?"ƒ¡Ia)?ƒ6b¨ñÅ?çôwñ©%(?°ÉLdø÷?Ä2ð˸-?­}AŸ1´?¸7ڐCh?¤¾ë8'¥?ïó$X‹²?Sìnºo?P}«êœu?LhŸ
"p?BsE¡‡ãQ??w]ÙËË?ïUñS2‹?'-Ñ:ø
?ˆì"ì~è?Šd`«%-?—´è®˜m?ƒÖzFW¯?ï<f'Xê?'kKαˆ?@EqL"?~ˆ¤ùÑí
?à;Œñ‡?lñ¼ʐ?íÒ8+¾?'IÆõ&Æ?¦ÀJ¼ÊrÁ?‰6Gya ô?˜8iɊ\—?‰l=LAAGN3FGL J1722.7+1014@@m ‹]@8M@LzÀ8ˆéR>'5À;86%UúÞ¿æä¨Y·¶@˗I]A$@`Ÿ l1,¿ßýZ¸w+¿çÃÂÔj>Ò¿àqaûƒÕž¿áÓðÇË'©AGNfsrq?ïý#e ¸?/ôp5L¥?kZXæ³?\Õ×[et?2è,s'ç?-¥³ÐÙÅ?﹆¹¤?€ ÂÁ§Èæ?lfWþ'?këƚÖ?u<H³µ"?y7æíÍ~?ï1Þ"Š™?†Ì˜j1±…?~H^¸M?q¾2ÕìÍ?'J¬‹3±P?"=ì†èÈD?ï¢0;²Ð?}‰¢"ƒÏ?# v1í•?$Ÿ¯_ƒ0_?‡%o1Xk?}l%ÂòÒ?ïþñÝöÞ?™éZñ?	e'×]ª?ÖJ°D?›»ÅSu?bL{ÂIr?ïãò-âï×?g!>Væ`Y?W Þ½©.
?S¨ú Ì5?`=b¤‰¬?aïc·tÊÒ?館?Hõ?s¥(
cšÕ?pªÞorbÎ?egtM?zÿ$Uže?nè«?~Y?ïì€ßìí²?Xý¼"ªvS?
%dzV¸?<'vš¿>?cëw
º?XêCÕ¦;AGN3FGL J1722.9-4529@uz!@W%À«"ÿٔ†À9ÍSÛIÀ:°;C¢ìÿ?ԋŽ®Ùò¥@
­ñœÆ@ÁeÖt¿ã@4}áb¿éÏ"¢¿³¿ÙwÜÛb½¿ïÿîbHÊtOTHERspp?¾ŠuØQî¾?Á@	ðÄ£³?§_Àxä>ð?±-î¬+Óª?긵=0"z?Å>	o<Š?ܑA0vëD?ΠScªÿ?ȓŒ{ñ4ƒ?»ª=žÏ—
?×$ø}™¼?Èë¿i•x€?×Ì꘩sp?µj"«?«´?È8J½F$°?®ÿxGn¼?Üð³z8?¸ÿbÆ$»A?ÕV">¡Ùã?Á•JÙ±Ñc?µN{ðp¨Ð?«¥'"JWñ?â«b"?…?ÃVҗ'?Êžû/O?É|UuFW?±¼Ï1^¥Z?¸¹KEx°?çH>[
?Í9Ußä	]?æ"ƒÍKð?ÉÓfâ르?¿ìÛº?ET?·ø£þ?ÇÛD…l?Á")‹GNý?âãÐýª?³;	¢]eö?ŀNd<®?«˜ÒgÖ?ÎóB[³ô¨?¯O·=ˆ¡?ߗޡ"'?º÷›S>Q±?¸v.]õú?¡"¶N
ݗ?ÚgÓ&áŸ?¹•»œ+wÜMIXED3FGL J1723.5-5609@të¿çáüÀ&IFÿ˜ÑóÀ9ç**¾ðÀ;VB7²ô´?°_홃Ç@Lêik@ñ ÀTnl¿èæ¯æfÿ¿êò­Ï†}¿Î}$ƒmj¿ç×a"¯­WAGNbcu?ï¶ÿ[­?}­`èüm?GVxÀäq™?JiÕ5"9?€ÊÑùžZ?\ù°4?î\¯ú•C/?«$Ž	*'?†ðܺZ?'ñÄz"/Ä?¤xÉOË·|?¥jlQ·Ù?íÖUÔÊ'?œ,að¦j?'!YŠî'•?€g;üÅè?©‰õõ€™D?—ð̐¤Ãè?ìëœþLª?¨Ýn?p¦.su'?rÄ®<J+?·˜¼j
'$?§cÉ®6?ïÏHP?…f÷zߐ?I´~¬Üšv?\ãQúo?u%HJÁY?'º¯çUc†?ïQ.wJ?–ZBð…?tp¾n:‡?w;³+?Âê'Qù&?'}ÏIÁ?ïFS"´,d?ƒBrÆeq?}E3¹\Ý?i «Ò?Èt6áþ?€¯ZkÉa9?ï–×Xè?ˆŒñUóE•?pDƒð­?`ßíSf—¬?™wG$Ñ?†}ŠrÉÆêAGN3FGL J1723.7-7713@s»	 'RTÀ5˒€ ¤PÀ8ê̵O؅À;nÐ6䘛?í¢ز¼´@O·3ÞSÞ@ü?¶Ï5¿åQ¶†íοâù)Î'¿éØ8Уhr¿êú¹…$öAGNbcu?ï°Y¡ÿ;?¨dÚ
?²>o"ø?~Œ28n~á?RUXÔ,ê{?Kß&ˆL"Ô?îðÌÜśß? `ùp
~?€´@m:6?zhބeðí?™âŠ>Ö×?BÚÕ÷þ?í#üÎ67?¡Ó|½‹~]?®$<Шg?qћÁüŠ?Ÿ7îRÖI?;*M†p?î3ZS™ÁC?›`Œ•vµ™?'³`úr¡?‡ëºYÊÐ?¤	zg~?˜W¹¼?ï×£¶â?n³"ßEÈÔ?qÕϵthu?m}":6ݍ?BÅ7k"?:	Œ¹%?%ªù,?‡Ö¼IMÐ?j
yÕâZ?cb÷¬Ùl4?V"
W?"+Èhã'?"?–k'0ê…?žŠ	Æ·¼?'‰¾ʏ?‹«?}ßþF±.%?ï‹u_[7è?{ôÉ-?…$?xq
/§±4?ii¼JS?€ê!"Åçx?vlùAR›AGN3FGL J1723.9+4004@P8Z€¶–@@–ôÿñ½GÀ8ÕÁw.4ÇÀ;¨"Æ£½à?ó0ºø¹å"@¥³ŸTD@œÏÀr "¿äs°¢"¿å›{4îc¿çÂá_'
¿ïÿÇ/ß_AGNfsrq?ïãÅ"ù?l(p*@5œ?\²ÚAÜA«?a"W$Óî°?[Âßk¾r ?b³
Sèò?ïu¬¯´?†0R¥‹¸?€°«¯[!?…G¬…è3q?äÇzÍÞ?†]Iàˆf?표ŽQÎ?ŸT­ÒÕÞ?©4ûÒwEW?™Šb§¼ˆ?›bvåp?*´
Ø£?ï,M·í?•O¹8!X?Œ1y6ݾ?"ÍLˆö‡?ˆ»E›'©¶?‰‰þ›üËB?ïó,¬u-B?VxŊ…¹?Oӎ<Šþá?Pµt"?CyÀEÀx?DЇ€É!?ï¿YÙÆI?v–'¶{¦?o»Si
ԍ?f`ø%[¨I?puîd%?p"ÄŒ{<Ñ?îom´õ{Ô?–íL6Hî/? ``lñ(?ñQ§Â›(?'QF§UÛ.?ˆw"VM?ïÒTÀ™?qG+.?nÄÈ¢•É…?g»# ¤Á?^oŤÖ3â?e°}ŀbÉAGN3FGL J1725.0+1152@A£_ëøâ@8|H 'ÁçÀ7ì=s(À:½ ùt˄?îJh[´×@…¬àa?þ*?›Ü?¿æë'Éý¿ÞÓÔmÕñd¿Õîqsp÷¿×e:´SP¬AGNbll?ïõ~a&Wû?Rëöþ…Ø?;;OÞÕ?9Bæ»Õ"y?Lhô§$Éf?P+Ëõ;?ïU|¯xº? (tÅþ7?tÀ¡dL?€ô6Ûú¶?‰!ZÏA?›!*>G,?í»È,¡k?¢K—†ƒ?™ÿéë³×?''i¦A/¼?§Cˆ°‡)§?œ5HT'?éٝ?°CÁÈ»?¢ù=
ê‰?Œ4b^èð?ÉË%Уù?¯"…ï©×»?ïû|÷çœ?;	_DÓà??,~¯Å…Â#?){"ÑS?5Øç"ìäl?3†'d5=ü?ï«ak"{?‹×1íX¿?rœ|»¥ý'?rû¿Q'µB?w²Í³Á?…_"RFŽ?îƒá¸†°?™ó,^Â?•º¿t˜°?'WÑ¡hˆ?šm3:
D?'¤>­ªÇ?ìÕpü±/Ò?™?7Ãþ¬?'V\±B?€Õѝ¶D?´¾á
0Ì?—Dw~;Å(AGN3FGL J1725.1-2832@v^"@lÚ@û6à÷IÀ8·N?(3üÀ:†–UAzõ?ó³'6{@;e[Ï_@Ìõ U p¿äÀ€æDm¿î¿'Þt†¿Ø+¸ëny¿¼Ç5oùbOTHERspp?á?²gƸ·?Ï¡©Þ`H?˜0ˆ(Æ]?™ë©¥¹	7?Ûý'®T!ü?Ïÿu h€G?ëÃ:°]´?ÌÕ,¦ÀãN?"à¥N?˜™^µD?Á×ÂÒ«'œ?ʓ^¬ˆ´š?áhvìÛ?·;3ñiÒ;?À%ÇæÔ?¦ø¼û£™?ÕJDXà?µLŠp}?çV;ݎ?ÄPøø­?ȹò'q?Œ;C';?ÐÔf÷'`¹?Ããw"àG(?åóIÌ@¥?ÐûCtÁ?r?˜TõƒWìY?›³ÅóGh?Ҕz1ÿñ?ÐÑmúôW?ͮZW?¹weGo·?vŠô÷ùu?"¸8¬tÄ?¡Ñ!È·\?·²ô‹7?藞ɞ?°¹/•…F?²‡X샵ý?Ÿ§è6Á¥U?Ä]ØbØy?­.ébß½?ëé¹ø3ØË?²"oo4Ò?­áC4.Ç?ŽÉ£Ã+GÞ?¼¼tfþÖ?±e'ßÞAGN3FGL J1725.3+5853@Ußϟåãõ@@ÿŠßÂr×À:cµ±þÀ;ïLñJZ—¿éù@ö#Ÿ†)@no?þȝ¿á ÁCà28¿à«¥Îö¿ä/vve¿ãñÍhAGNbll?ïÏñ_{'?©Þ¥[Q‡?Wt÷â›ßN?‰ãÚ_¦fƒ?r*A^zwÖ?¤.""FE?利z¯t?"(Iþ¯?qaï\7o?mXL¸¿ ?zÏS¼Á?(Ÿ¶à›?ïmîÀ'Í?Š¹­çT?{{,]Œf@?ndkIö?†Æ¹½oov?wfÀ3b?ï·&®{º?xßjÅ®èç?Mñ;ãê'Å?K2›Bàl"?€W@œ
û^?wçüMJåò?ï3ï8\'Ó?ÂØ¿\ªXŒ?vÅsô
×´?¡áÝlWA?"лï¯Ð¾?½l¼Á¼ÎR?ïàBM,ƒ—?j_ý¬–³û?Z"œ™ò£?TÇ"üé?bsäŽÂs€?eMýŽ‰ŽÀ?ï¼Ï≀%?mù×>‰?kcÒC
?V´·¼¡.Ú?t\â°l ?j]ƒJ™™?ïô$B]%S?R²o2x²H?&"¦Ü`?4÷c~¹å?Täû©«¶?RB^Ž¢'AGN3FGL J1727.1+4531@Q܇ Q»@@©÷¿¿žÀ8¢Ëlz|žÀ;¯ß´tç?õ`]æe$G@{bcL@¡\3\£Å¿äZÇ´Š
Û¿æƒÿíFâ¿émKŽ¿ïÿ{z
§AGNfsrq?ï쯡vek?X։VðÇ?XÞijî˜?R¼ÐÖFÉ?K…Zb/?Eñ÷7­¼?ï£ò…e|?—k¿ÝU`?›sïc?Š9<Ç—´?‹û—‡ý'?ï´;-?îv1÷¯o?•¥_íȽ@? ½ú­ù?',Ùœ$—?'·-L*?…ÓČC?î•÷3[TÃ? ë}08î?›êÿ2
?˜ÐLY?'V‰†5–?"®j"?ïô~',<õ?N¯þ¸#?R/ˊ[§?K+îŒ6ß?3O"n¥ÅÌ?.þgì+¡F?ï™f¬Ã~+?ÍàÒùñ£?{™ªÜC)¤?t$YÞÇ?w²þ£Á1)?wOS-Hˆ?îÎR]^Å?T²žs)5?š
Ӑb?Š
¾'I¯?ˆu5B¾'?{kôgºõ?ﮜÂ\Ë!?K<'CEb?}æd}ùð?uUiFö¦?e–tæyÎ¥?r0¢¶AGN3FGL J1728.0-4606@uy¬¿±[WÀ
€F6pÀ9:¬.Ǔ¨À:üº·÷R²?ÖQœˆj@
×i0EB)@x?V×þ¿éÀ	oëJ¿ß<Zú!™®¿àeýö:"`¿ìÁ°~ã_áOTHERspp?Ïé;«°P?ÆÁÇFaI'?äù«‹š¹?ÉÎfº–Œ?¸`,I5ÞF?¶ãQ²G?âD…\!?ÌVH…!_?ÃÀgÓgµ`?¹>ë•hF?їÃ"
?Æ=*Ì(?àMÆÜ6»î?¶M?'º?Ó8þµc_Ý?³DÛc?ÈVç$^P?±fnøDñ?àÛÆ9à¡?¶€S¸÷ž?¾.'–s}?§Eö|›?Ø<¤
ï_|?¶ß/+å×£?ØÉ·X
Fð?ÈÖ§hôi?ßè*ªè:U?Ê1ÐÛWݕ?½8wïêwò?º>>æ*ýì?ꋈøw?ÆÚÔ¯?±±ÇÛá?ªR¡b:?¾Õñúåã?¼k¢‰à¿?æ«Àb±%?±¢w‰¢Â?ÊQWû-w ?­Cî<aš?»òDœ?¤,ì9}
î?東Só?¬ª	Š`?µÆV,Ç-?—Ùvt°ä?ʦž®]?¨±¥;6­MIXED3FGL J1728.0+1217@Anž i—s@7þγ#®À9u;â.]áÀ;= 8Ûê¿å´ñÙ÷'®@ï¼C͈@@w˜¿ÓNŸ~ú ´¿æ¬Ó;ë'^¿ã¦®Å¿é ›Žf_°AGNfsrq?ïô(UK?h¨GQ	GP?L.špã`R?_#Sz§D?C0ª!Ó8?[Í"0Ï$?ïžâV óë?‡ð¢{%ÌT?r<Wµx¼7?oXèös?~R}"¯ö/?"£¶ƒCÉ?Ûå»Ó?"û?¸
b?˜­:03–´?'â˂C?"*X<XÖ?…lÄì‡ü?î»dø})Ì?'ïÇRÙN?X†'g¶q?SáÓ­±:Š?£…{摀,?'tTjÚL9?ïúcæPÎÇ?PÍ«V?@aaö¶"˜?P
~²Ói§?(<¡¥?'£âÏé?ïÝëX±¥ˆ?lτîæ?\å O?U,²Ð?d´â渳?fJPIY;a?ïB°"»l?Œê0Ç]?ŽÓœäk"¼?‰J%¼GÜr?€€=ûײõ?vpó'¦?ï©
¼šê@?pˆÎçÍbÙ??èq"?4X'¹W;Í?"½P´Ì›'?p=‹)SmAGN3FGL J1728.3+5013@SE@€"Ð@@ÃF߸aÜÀ9!EºtÀ;~JÏ1+¿ü=¯
@ìuN‹©A?ÿ[–~²­¿áÛ0–†ûÿâ*"Ô€Þ¿ÖmæÚ·i¿â$í|ÓAGNbll?ïõ£©žš?KYË¢ƒìr?;a²Úµƒè?3²"aÉÈt?KÀƒÞà?EÉׯÈ?ï©´¨Øjª?ƒùõ69Ù.?r<é՛!_?oLžª¹×?xèÁÆn™Ó?5.˜VÜ?ï__(R?ŠÍ›¹5i?‡;À×h_¤?{Ã}a¸SY?'ö3²æÅè?ƒXl‰[U?ïW&!IH@?‹zÆ7	ì
?3I~È3À4?8äZs'ÌS?"ÎÚÚB?‹H^eLF?ïú.,Á²›?:'ˆøÆßX?4[æzo@?)®ÑÔédÕ?:2³—,±?2¸½]i?ïßòPêÔ?hï£~,PJ?ZU՘üýH?QËÃ'©‡Ž?bâÄU
é?dՅß!Àô?ï‡É¶J‡ì?v
XhVí?{)¿â²®?o¶)y¤È?€x²ð2ý‹?gê¬ÝŸR?ïÛJ|ù{?f4ÔúiýC?
ZÁa;Z??*N'?r&>Y2E?f AʕÜìAGN3FGL J1728.5+0428@;W¿PãG@4sÔ Ö¤½À8îdüÀ;Cí\M?òˆB+ž"U@Ɉ$Ì@ÀÿÿÕâ¿ä«ZÌ ÌÌ¿çÒ{•w ö¿é"i+üÄ¿ïúÊ;ÅJAGNfsrq?ï½ÙÖ[Òö?zgÔsRÛ?t@s´)?tUüÝ?i¥B~±Š?eÓ¢dÕ~?èÂÃ]C
?¾Ùúo®u?ÃvÞ̲(d?³Õ¢ýD?²ü*?ÔR?¶Á±pèÚÑ?íŒÙÜø
‹? üWSë@?¨ŽUõ~=?—qåüMã?ž1§º;-?';Hd¼¦?à¦,KRl?²Ž‹øµø?ÔÒâñ&s\?µ—æà ?ÃÁ‰ …Ï–?¬@°ÎƒJ?ïèðç´.Æ?`|lÉðr?aڀõÌàð?\-ºí4þ?DÒ]ÔPq?@Ûu•S?ìYÁñì/Ø?°×uX'ß?³_
oÇ£?£'00ù?£¥Ì¾ñ(2?¦qN¬ùWK?3ú$ì?'¿Évô?›`ãtÍë?ŠluóB?ŽŽ¬
Œ?0¤¬(É?èÓmAˆ?¡â{tec¤?Åpåßs?¡–g*Ê?®¹E™WÎu?–½ŸãS¯§AGN3FGL J1729.5-2824@vhË@p2˜@
!ç@–sÀ8ÛwˆÍ™{À:¬¦]¨R?üó…†QŒ@^köÝ@RtÈ©Òw¿ÊÃõùó¿êÄȼœÓá¿ìd1Xh¿ïþûB0&OTHERspp	?°QóZp²ò?«ùÚÜ`çÂ?éO^ü©x?ÇüéÒ?ÃÉÈ֞ç?Ãä䮝?œíˆÖ"&?®•Å6›ì‡?áX¥̸š?ÇZÀš(N˜?ÛÝ5OÃ?È?ǂh®?ÈZ½iNð?­÷ËÇ÷Ím?à‹¨b4R˜?´YŒ‰v?Ò»¥Üâ³X?³=q.ÿ7|?ª)ªcåY?šAëR‹øx?åv"<vd?¼±nÍh(2?ÑÏòQý´Ý?º2\‹
$?¶¹ÿî'í?·(x?è-$M½"5?Èsw¯Aª"?ÃîßÉK/v?ęXÎo±‹?¶S¢ÏAT?¼y.:âe?â*rSs^`?Á¡¬ìe×?Ö2¤öwŸ?Âòñ'I¶O?Ó
fÇp~?²xÆ¡¢m?ß	»É!û?³uíÁO?ËÓ×½œŒ?®Ø&FÑ?´@'‡Õ¶{?Ÿ!–R½<6?ç(ÜhÝJZ?±8ª*?É<E˜2Ü?«Y5ŠØ3ÿPSR3FGL J1730.5+0023@7ÄÊÿm3	@2-ß6[ÝÀ8Aðþ}=À;ÅJøK×?𭷀µG@×6aæÏØ@ƒ@7'´¿ßùnurý¿âh!š*¿âqõvlÌe¿æ'>×+KAGNfsrq?ïûðý0ö?6 YÓ±gÂ?*zÓH@þ?#õ¼
?3BûÏY?/áÏüïÚÝ?{ô©F?†Ý¯:n$œ?oýĹõY?lágb‰'Þ?~—C,=^O?ƒOVÏ;?g¸î?»t*?‹D1×?KØ?2·n?'éâAÒS?"¶	÷+™W?ï¿{´	?†¹±M?XËsI6tm?a8}Wi'r?Œö²¦[®?…›j£8´?ïýéù"'/?$à‰á>?";3˜?õ·?Çdͅ?Ja6"o?¸ît\­?ïÙàî0¹u?m0Ä9—ý?\ĦfÊM
?TÓ úғ¾?g¼¾c‡Ì®?fö¦3‰°ö?ïw/'Gse?€"Gºœ¦?€)ƒ}¿k?tÉän`Ò?'
—çÊuv?uƒlr£B[?ïÛÿ%DH?f¼ð 7ý£?P=óò?6^?Fð³Ü»c?káàðo8"?e%q﨏AAGN3FGL J1730.6+3711@Né"åx•@?\
ÿ7ƒ$À:p¨ß‡ºÀ;ÐaP?í±½k[@yò'>N@³À€8Iž?ëQႢ˜W¿å˜tÄ´5¸¿ÛIlΒþ(¿æüŋÃu¿AGNbll?ïä'4[¸t?cé岄ö—?X~ÔÍÉ`T?ULj–;¶#?^\"'è?XM›øš47?íèZiØá®?°Ø]ç¡@U?¤_OÁBÝ?§?ã­ªkÑ?š6"*ˆ®?¤Ÿ|>?îsôú€5?—/4+§?™"ÂåÛK?¹à½Ã»?—ìÖà>?‰^œ€DW?êN4­uˆ\?´¤Ñ½ï±¡?µ÷täU
?©IÐÍp2X?·–å¯þ¨?®GÔQ'È3?ïôŒñâÓA?W÷Ÿ:õ?H_' ê5è?FZ-W¦!6?Em6?LˆÙ¤¸$?îú†gë»? Ê›9ã[?"1΀ÂbZ?˜Gòx|X?Šúß'ïèn?''t® k?ï=V—ç<æ?‡öjLqj?ˆ^¡,'SÁ?~ʾÆÌó?ˆK¸Ýy×?}³XêÍGØ?íëGù¶1L?–ÅHÈ;…¢?§û±¾]Ü?"#']=¦?'ŸOíº>?ŽÓG´KUýAGN3FGL J1731.8-3001@vW¼ ?ÿC^¿S À8~ŽŠqÞjÀ:…‡ú4ää?ðD%'_
'@
®>lL?ÿÅ*A*¿åf?²ûóß¿ÊKf»uâZ¿âD˜L׿á6g\IpÑAGNbll?äEˆ¢üCÞ?˧£ÆKÜÖ?¥×M¤$l? ƒCf¾V?Ôº°}?ˉ€OyC?ÕîYDZ?ÖR9]Ĭ?¸Êaìw?´x`ޘ%?á﬚ʓ"?Ô
e˒?Û
â$U}i?½|	CºY?¹÷q_?‹?¢Xd
¼S?Þ³ßÿ75Õ?½»2[Fù?Ù·W/fË?»3ä•ã£ö?½&å~ì¼y?¯±tU¢Ô?Þÿ0Ij?»ì°9ež¸?éØþâ?Å֍0æ¸í?›¹(›£¶³?›iy@]¾!?Å(rqÙÙr?Ĺ6ܤÊê?ᮧ3á?֒áNd"?¶–Æ4}H?´B®_Ö'µ?ÖþC$Ëo?Ӂý¡O?æFàð×TK?¸Ëˆš#õV?°üótñƒ?›.ðºZñ?Îf'*+?·5Ñ9)R›?àè3šƒ›Î?¶T¯='f?À£À{¨t?¢
Óä0P1?Õݸ$Á+?³PŽh)MIXED3FGL J1732.5-3130@vDüÀz®ó?ð?8?®ŠÀ6 ?û˜'3À:3X–š@
u9ó–»@FÿÙ> $?ëÊS0‡9ù?ïÿ(#,!¿ÂwÕRò.¿äƒÊ'´'‡¿î3&‹ÉPSRPSR?x"­9F?‡h& vÚ?épª­ÆªÒ?Îäc&óV?É|?áÂRJ?΃(˜>iŒ?N~Û㑈å?|ýZ¿ºc?êΦ®*?ìüs"³g?ħ'Œv?Ãv"f©Ø+?¢MÈπõù?š7n²?㎭ÒÙ?½¨µ<£»?֚"®´;?¼ØÒÈ?MÞd<ºµ?Mč6øi?î`Ò~E2î?£EB¾V?©~pŸ)šf?£8Ësgs?x©º‡Ó"?Ž€Y¼H–?æ
í˜k¿?Ò³Ñâ4_?ӈY:ƒßs?Ò 2¢6¶?d«¾ûùï?'ݵγz?ëq¡Éÿé?º· Ýݖ?Áæʍ5à?¹›â3¼E?¡CX?=Iæ?š
‹uô·?äTÏ uR?¹nt]è?ÕªëZE_Ÿ?¹@ÆY_?S%Žå̓
?IB\p¨Í?î`Õ¾õ
?§__IJ?©YwHåG?^("ÖPSR3FGL J1732.5-5048@u@i³únÀ"ÖÃà'TÀ9}:í;ØÀ;W
V›H?ÔÂS*ä@$QËú"Ü@Fk€V§'¿è¹?H·¡¿Ýqtºf³¿èú4È«ø¿ìê×ýêPSRPSR?êÌÞö£"v?½ŒŒ]úd¾?Âsªu'‡?½/C(b?'Ë£Ýfþ?#ö'½Yô?è2$3~)?ˁ}S|C?®>ͽ"ý£?«‰™
AfA?ǧ¼‹ÐÇó?Æq£æ.?èŒú¼£	?²sª{üì?ż"¢ˆù?­šÌ0Ì0?±Œ¶×ùîÇ?›7ý@T?è5rFT´I?©zÓLAä?·š=¹úD?¢öùoR?Ã]	A}?¥·àÁ÷0Î?ìÆe`ñ¡1?´¿`"€µN?·uHåù£Ø?´-?ŒqÃ?'¼`"¬Lý?"à}ÕØ?íͧ×ä?¹÷Ö	þ9?˜¥¿
Ð8?›äஇ]?±p#²˜É?´
§&Ô³?ëz[·rã?§aSétç?ºì©‡´{?£ªæ]'c?¢€ñtOqÓ?Ñ²]âh¨?ícü0_Ò?'‹Ê‹ð\Ì?ží˜¢¸L?"-êx.ÿ?ªIp¨²ÜÏ?ŽÉØgöÌAGN3FGL J1733.0-1305@(÷ÞÉN"@% 6^`ÞgÀ7'ÎuCxüÀ:¸M`Ûâê?õ5ÁB€D@Ç2]Ë7K@éð»>"ö¿ân¿«œë¿æ'Åeòš‰¿ä­cÐß׿è*»¾—ˆAGNFSRQ?ïéùó˜àÙ?bY¦Êç"?PcuˆÌõ?NJnœ,ï¯?[òµj»O?]áû‹8Ç4?ïMP`ž.?œµ4 ]½|?r«¥Úuyû?ƒN'Ê!?'«
zðEª?™u•§sVL?î"1CLŽ'?¥ÌùZƒá?•×Ê×z?Ž->Uõó?¢ñ¹"Æ,?•Ù€Hì>?ï҇ҥ\y?z÷$6…–?!¿¦Ø7¦?+b/_À
A?v3hʳ.Î?yüHÁŠy?ïõgš»O?R‡+œ0ö?E€ªI›Ûj?CkRЖDZ?Dàé×Ð$?IÁ7ý: Ð?ïĖ žy0?€fؖJä?]àHê$'‰?a{PhP^?v<WMˎ?{ז%X¡?ï-§Fð?'"EænR|?‹UÜåÐ}&?ƒÕÿ6û?Ï\Z†n?‡6ñ-Õ%a?ïöXe¶ö?YÇ^8¦?¨sÖ,Ú<? VâÄö×?Q´­Ã['²?XÞý"+D'AGN3FGL J1734.3+3858@P"ÿÖåU@?…_Oñ°À8GuÇ,yÜÀ;m>m#
?ï6¨ê¼@]®:æ[@€…Zmà¿áj0]Égp¿å­è…ù¡¿ãÁ5,»''¿ë_š‰ŽAGNfsrq?ïôÕañ·"?NüÇ»KoÐ?QÒU‰\¨'?M0ÎÀÂù?2™YÒÐ}?(ŸÇ<T'?ïº&	²Žç?€^+È|µ?lä K`?mp)!oï?tz´¨pþl?wŸV"£?îÄ·"@?'ƒ†Ovu?˜'Ôµmmh?Œ"ÑÄêfw?Ž'Ž
•?}Ú©Nð"?ïì",û‹§?lª·¶©ŒŽ?):3õï¬ù?<?7õ!1?bJ/÷†>?k×ð«œûø?ïùÅ;3è?>䕂?DFr'þ?:›'	í}?"'†P½$W?§ízö¾l?ïãùšòEh?h$	[à±Ê?XIŠ[ºÆ?T™ä1¶8
?_þ€üMC¯?a—öïôŽÅ?ïVeŸ ?€ýŽ…Ç.B?‰UÕM
Ÿ²?{2"ìtA?%QuùäU?lŒ
Àä€?ïüÇg­Ž?CÊ4ˆÀH?s¸DðsÈ?"¯ØwmãÛ?4jΝ%
?Bšl?KAGN3FGL J1735.4-1118@+Æ!à$˜f@&sA¿½ð'À9OsGö8×À;4žm>¿êšŽÇ-¦@ç\20@@O¿Û͜¿Ððs{ÞÙÑ¿ëºeð°èҿΤf/0¿ØøáÎ;·¼AGNbcu?í¿x%€˜?¹ùÞ#ëS?P7ú±¼¬?PBÑ(+,?·±'î›#"?¹ò¨q¬HQ?îÊñÇõð?°;S
"Ÿ?uÃͲ´H?w•íTd*×? ˜ŽÊ¼.ø?¯Åó@‰Dþ?ë!`÷«a‡?®'X0. C? b KC0?ÃönÇÌ?¾Ãèqf0?«÷~¥m$€?ì÷d­ÿ',?£ÍWç;›´?9ý®Èœ?=ꪝW?¤?¸+ǔ_»*?£ÈBA¡"—?îa~u?´¾üžn?F†$/Lø?IKþß[ñ?©ŒåŸ4@Ø?´»	6ý›‹?ï°ºd±}?"ò"'i¬`?a–ïoŠäŒ?^/››å½?~×H¯þ×'?'éŬI+?îEâV.Ú?–ê'ðl¶£?wW<ŒT5?iCFðå?£f/ڝH?"wHrà½?ïy.L!?†åÙ¿øž¥?35fצA?$üWSD¥?dÃA(?†ÌE\cTÏAGN3FGL J1736.0+2033@F@L j@9k>¿XpÀ9rêUrùÀ;P…Ûv³¼?ð%ä‹Zf©@sòoɑ"?ûŒ@ Y&b?ïþI™HˆQ?à6¦,Wª¿Ø^~ŽXüN¿×–fUÁÊÞAGNbcu?ïÎ%öÅÕÉ?vªŒñQÔ?rkµìo¯,?sDõ(9È·?Z:‹›ñå?`CK†÷Ž?î–tæÜÃe?²l\;›P?–No´ÔL?£C˅õ®á?–âów'÷?©¨*¬×?íÅˆÆô­?¡qcµ%?¦Ž¦¶ão?™
Ó¡Tt?¡UºõeÆ?"ì`æʤÔ?êõl›´¦æ?´K~	+‰?µVÏøn?®'"Ö|©?²ý̆àb?ª÷ãA|x×?ïç*õè>?d!2Ð1½?b±ŒÔ¶ƒ?a§ã.ôP?H'Ä=ù?GôÅøå˜?ïUé)Šú?¡6aÝ\ëR?‡ù·ÆÐ?˜%KDöî?'Œ îÓ3?'¹?wZù? äÛ?—)¡!îF?šï"tg¨?'A®'œvÎ?"@7á?`î?Ž_Æ(É?î9@w6?˜O­8ôˆ?¡%"oÒ?;Œí—¶?•Ù±Ã¤2Ž?'•M:¸'AGN3FGL J1736.2-4444@u˜¨ÙºÀïLßזÀ8ZHùn‡À;S‹'?ó1£™D_@ˑô^·@'`gÁ¿å±öy|Ä¿àÀЪ§Þ׿æMÞzt:d¿ï#û½{ 2OTHERglc?<¶d?ªu‹§¦h?ì]Ÿ?ËÇê?¼`ï¢u?µÑöÜ¡?¹Ãxû"`u?ˆ›*JÇ?–ˆôMÒï?çŸd‹è"‹?Á܍n+ñd?Ïø»0JÔ?Á}Ï=Zl?Óò´dÃpz?²uH¼P`'?ßËzF
z?³ÜJrñ¸_?ȃ¢ªm?«Þ[»H³&?¼õ[ÐÐ?§u½d'""?åüLQðÁ&?¹€ÌµçU?ɔCŠT"f?±§Ni©ï?¯hõő?¬–I-•X?ë±kJ%èó?»½"&–uU?²æq2¤i?¶gÔ¶ÿ?°Ÿnƒ?¢'•Š³{,?çëœàdÈñ?½ÆÙïÜ-?̛x›6ª?»¼%"?âUæØÜû?³šÚ;"8ƒ?Ô"¨v<?±§kÚ½§ö?½ E/_6?¢˜JQAm?ÑdNÝø]
?­¥Ãš/Qã?áèëçDGX?µŒF‰w­?œ²¦þ(‡?§;xy~ëMIXED3FGL J1736.4+0634@>EÑ q$0@3¤:?–îÄÀ9 QJuoÀ;G›	b@?í10âKF@êßp"eù@فà?pX¿è'%xyR@¿é
ÎM$¿è@doÒ\¿ïþ÷‰[U^AGNfsrq?ïõkÂEà4?Múl7I¹ü?K.\ö'z?H.'6P"?>EÀÙÞÎ[?7':%Cõ?ímÜZÎ?±óã﬊]?¦^Á²`'›?Õta¨q?¢Ð=T%D~?¬ªË§% à?îH´	Ž'?˜'Ý¥œŽ? 'X£Câ9?ÕØþÎ'?•äÊϯpÀ?‰"L·çÙ?çyœ»¯e€?­M POË0?Áüܒ›+H?ªeãz1v$?À°~§>¸?¥øŒëR¢?ïöÀ­žx?Mï‡à>Ÿ?M¦"ê¦d-?KèJÄ?-\š'Zu?'·Ø.Å??îìJƒ(`i?™,*K?"?"_µË"Â?…VØÙêOf?Ž-ó'^^?"ˆ)Ç´?ïBh@—[?…È£fYͽ?"4Fك>Ž?€v÷'A–?†FØ2"Ø/?teÈÆRÁ5?ìɗÒÞÎq?"'ˆo<Þ?°0,RZÚ?]é"p²?£*/Œ1=?È?c1'AGN3FGL J1737.3-3214c@vD*Ÿ{Zê¿Ï*À1äÀ8kógkI$À:|Oø?óÁwO>'@'ˆíNø@$H¿aL¿È4ì›Ê u¿è6U'Ìc¿áȵ¥8¿æÕožŒÙOTHERspp$?Ø¤.cŽÇ?€Ø*K÷†?™Z…a~J?¢çT%…Æ_?îíȃD¡"?¥·^¦~"?¥Î!naGô?±šÄÔ}<¹?»5ƒœ=ì?­Ô‡ƒÑã
?ë<mw¸Úc?» ê}¯$¾?½5·œäÓ?¦©‹Ïß?¹ð¬II ?¥' ?é¶3ƒ:2?°‹ìX"|à?ÆUN.>àC?º«ÎdýZ´?¬õn×y#,?¢–ǽzf§?è›U†øµ¼?½\}3Sâ?'ÑÑÚ­Ôó?'"FšÑρ?ª`¸3…

?³‰³¢£;V?íËeíÖÃØ?µ—禗~?½ëÂEà4?èﺄî?ÁÅ"Û‰G?¬â›Yüå]?çÑ?'-?ÆÃëX9c4?Ê«ž3²4?°$žµï,÷?¹LW€‰A!?£!RM9J£?æ+'½'¦?²Ê×K£9?ËOyǹ‰ñ?¹A~_ui5?¾óx%^;þ?£ùÏxôj?åM²‰eÖ?ºi¶Z£OOTHER3FGL J1739.0+8716@^Þ˜¯@;ñ¢@1HwÀ9§~b®–À;Ýî­È$Ç¿óÅΞ^$y@r6xâêÆ@7ø¿Äс¿ÔcÏÁ&"¿çÕ¬A3sl¿Ü
û˜/ë¿åŽ¨ê¢ÿAGNbcu?ïýá7›€W?&7Ù¥î$­?{†*ÀL?ÛPž¨Ê?(®Æ¶XEw?#Çý1ܵB?ï¼ÌnO‹P?€—lŠñá?j]ö*'ú?mÂó©1G?tk=aDž'?y?dˆWŠP?ïG¼¥•ÙÏ?'× ì?€PWÏÖ\»?s­z€…n?À~ÁÄ3‹?~"{æ&Ñ?ïûn#&Ô3?G£·Gæº>È/'¼¤h>ØAd™Ùs¹?B/Cž='á?GV:ÆcË?ïÿ	*K-%?m%ó"k?*ì¢ïø?iè/kL?Å@KÉ-?BdÓMý|?ïçYŸX…?c*´é%r?T՗ÐWx?RY[çãx¾?\w(½ý¾À?Yî³Ce7Ä?~S(W?yª%GË»?ucÙ$³?qºµU‡Oü?zéµµ÷Ñ?rÜVMV¯k?ïÿq ˜j´?w2%[°->©"b®Ø+¬>­fJ—ÉFî?¨ì·aU¢?hÎèJºþAGN3FGL J1739.4+4955@S8ß¿î—ù@?¹´VÝ\À8à±é·ìÀ;¨Üôb=¿½EÄh@9¿ím@tÔÿ÷«¿ã68š6ˆ¹¿ãG×æÂ}z¿èÈ¿%璘¿Û¢'ĹAGNfsrq?ïû›•Oæ?:Ý8«ìpb?3"c·Éo?2o¥îÞ´?3–¾KdÄ?,Nõ~@Q?ïÀ;ÚÝÃ?}»¢"¯¼?k¿-eó?oçù#ÆòV?rٍ0þ?tmS.ƒ?ïD½\L?ƒí^æˆì?ƒ͒ll ?tã¶LÈz—?‹ÀÛ]übü?y¶uúÛaf?ïùNłM?T»ËPSˆ>ó¯"o2ó/?¬1`N?J'p÷—?T¦Ý'K…z?ïýæòV¸ã?(Z;xZá™?"è?a? *+?þVŠ?Q|¿‰Ò?Qv£´,?ïç̀j¸I?e¨"ÎØþ?T¦U–ÁÂ=?S£StKÍM?[¾ª?J&?_50''è?ï¡pìÀø?q7øÞYWV?vUØ¥ü/?gJ17i¨'?xàq®éÃñ?eå˜ì§?ïÿ*^°?'æÝÉ>Ðý@>Ë6Â>Ó>{wYV"?¤gFõ×Û?&Ö|/ü{ÕAGN3FGL J1740.3+5211@Sム3Ï@?Ê.Íû¡À8|6™AÀ;¢¡€è?íú9wEï@Úæ1ø @ž¿\V˜¿â@þŽ`¿ç%ÇçØ
j¿é¥Oê<ãû¿ßÃì]$¸
AGNfsrq?ïüFÓV²G?2~óu?1aš3¦U?+ÿ%ÓH€v?)`i@C?!ÞÖKèí?ï½r)›¸`?~3XûÏXÀ?kҕîz*Ã?lÉ"¿6Òö?s] 9†âo?v0NÁ
?ï:IÂÁ±?"ó>W|ß<?…agfXI?yڈRž¸?Œ((ÿWØ?{óêA؊—?ïó¼Þ ½X?`e™·ž‰?Œ#©æ'?)'"1'é?W
	`??`ÆòÆÑ?ïþÍhlë?$ŽZ!vfX?#]¿µèÁ?óÕUü¿?"š=Ü-?'AªîÃÀ?ïä»m¡:š?i û2œÒ?V¨›o¨ž‹?Te§¬'?_à‰ XÌ´?cŒƒ:Ô?ïŽê#IÜ?vÉYuž/?{æxë/V?ob½äKtk?}ˆüó¸ù?h0¿U?ïþ?69s`ì_>ý
klz'J?	£Ùa¼'?#†À­¥î?5Q¨ n»úAGN3FGL J1740.3+4736@RÀ'¢Ü@?SÂÀ®À:gø[ÆÐ4À;ìP->ýl¿ðÑÝgú*@攸‰Hé?ÿ&Šþøï?çâQ]¸q¿Ù£»vc3¬¿ÛúS0‡9ù¿ßþ«íŸðAGNfsrq?ïüÇÛe/É?>8\À¦?&È•ÈS?"$ýAñï?,º4pŠM?:̉j³#?ï£úNBá°?†Ê"æ1·X?q¦±â; ?m´3"P?|\&äö°:?ƒ¡¨£Nƒ?ï_ʧW-?|—xnß`?'+F¾J?rr'mNË?…âg³¢?n¸1¦ƒ"?ï†h+"àq?†gŸ[`?JÛv+™dó?M#·£óu:?Œ¸=¿@V¹?…ø-?ïýÃZ]l?3³UW»»4?±\CÕ?c¶u%?&ñ³åMM/?1"¢¥7=[?ïވotØ?jœÉè×p?\5GmÍB?S‡N
¸#?c\Èʵù}?e¥
x?ï¤þ³éj×?hgV!³ýž?u¾8Œã?^ïÓ"<?w½çßÔ7¹?ZU
L;'?ïìI ³?]Öi˜Dæ×?$nŒõü,?«è·îH]?bnHØÂì}?]GÄ2™5AGN3FGL J1740.4+5347@T[O?Ù3ã@?ã$H¸À:h\ïÅYÀ;÷Ÿ<pÊ¿ç¾W¢:@
ƍ³\cX@&"_ ¤{¿ì¶ø–‡™¿ÝKH·Ì,¿Ðú&2ë.¿àÎ[‹Ó§AGNbcu?ï÷ݙp q?EÎÊ*i‹¹?1ÉQ^žy?,Cûj*̙?G¤ñ©xì¸?B9²ÌÍØ«?õÉ_?‰êí§ÁX-?rž;tŠ=t?t@Džb‰?|"ɽsŸ|?ƒŽ•¸:?ïo¿ݯ?"Y…J^Ë?ƒ£¦ÅÊw¤?q?°OÙ©?"@4¶[•T?~Ö a'Ê?句röB?z?É@´½?F,c­¿­?Fåúb2­?…}X&yê¼?yF	ሔ?ïûK)7ö€?5­qŸ¼L&?%QJÇXÅ?!(}pfÉ?:þ5­ŽÞ?1L‰=]d?ïÜ/Ô!ó?j€rµ¸â?]öAy•ÂÈ?TmI×Qòy?dÕmní?e©—Ýl?_TEÊ?sk¼–¼¼?y‹]Fýz?m5KWìvó?T9Œ—iE?e¨SžË <?ïï6ycÄ ?RãªÒVš†?3o¬l)-±?$°S闉?\·"svßû?QÕf³&:AGN3FGL J1741.1-3053@v]:à;>š¿ÊUNÀFExÀ7â¸ø²<À:Ò³–šâ@Kڞòt@ý¸§ü´?ôdÐvû_?ä-v€dê:¿ÝW¯¿JÙ¿å–œ>‡È¿ît>ág8žOTHERsnr?IáfKä?RÐþ­?å:â&{>æ?Ðõ.š¾?Õ}K³ý?Ðò¹*®Z?hÉO¸y¬ˆ?…‡DFḐ?Ù¸X2éXÁ?ÃLä·F ?ã
–m%"?Ã}˜Ù«-?—;@‰7?À?•	øþÝ?æp‹‹í?»ë²"o?ÒOI§êÉ?º=Md,?¤sWo
vg?žê1ÿ¯â¬?ڔ³]\sì?Ã{œesC¼?ánpÚnÝ?Ä ª²-Ì?KÿG²"ç×?XJg±—»?è&{=Ò¸8?ÍÁMlU©?ÏJÁË3g?Í»R5ظ?x±@GJnÈ?"¸J¬?áI{ÜÅ=a?¾´"#—µ?Ý
CE$!r?¿^5ÈíLÓ? es2Ø?˜TRŠø"?挻LKY?µ^|¬sÇë?ÐÙÛ‡®N?´UðûQÛÅ?¥ü2¤™²+? PTò™½?à@¨'b*Ô?¼ëwvÛ?Ü¿)\Uýt?¼¹aÔEMIXED3FGL J1741.5+1351@Bð¾@Bo@5¢Àu¦uÀ9äêÅX/À;'H¸?ñÁ˜H¶¨@"—G…@Í,@zÄl?êÕû]·t¿Ü6]`¤0¿æþ5¹['¿ê
.Ž€-YPSRPSR?ß/¨*<OÎ?Ï6.'«¹?ÞúK
?t	?ÏUŒ]Š¹q?`̪…R¤?™ÒTü$¶ë?ç:ˆ«Ïjü?ʌbŸmª?È ì:?Âó%¶Ùí?µë¹Ÿd
?½EÃ6S¬®?ä*i®x ?¾>Š1û-f?Ñ^C;WÞ¨?»u.ô<ÛÜ?¹3¥ŸNsÝ?¡ÌÓ<YuÞ?×¢ €Aô?¹½
7«,?ߺwKL?Û?¾*³"ü?ÁG(füc?²yæñ-ü?æü ­'¨?Ë	Ä(RHf?Ò¬JI,ø9?ʔ¹Šûœ?"›ÇPžïh?'¥ãøå
ô?ëDèHÃ6?Ãt›Èé?¹ƒúG,¯ù?¼k±åüÛ?¨©†ââ×´?³Ys¸S?êëÇÞ#¦?®łfÞB?¾Lø|å(?©fwHÚæö?¤©ž5¿èS?'Š²…¯ƒ?刍û3p?°€P°78þ?Ñ÷§õZ"?®P'_ÀZ?®ÿià¡ôe? Ô"K+àMIXED3FGL J1741.9-2539@ÚÜ QÚ@XÀŸ—à\À8µlC9À:m}F|¼¿¥²ŽÙ³KX@
ש`Œß@¥@¿ ?é>ˆÅ{¿à0àÍàž¿çÖësd¿Õ¸ÁÀ»AGNbcu?ÃÒ¨IñÌÈ?ÃU~þsõ?°·çeéä—?±¢ɍÁä?èôYªÓ[?ƕìÂFÈ"?áŠJbû?Ôaîü'Ob?­ñ–kö´?±˜¿Ž|®?Ú$¸3ìT?ғ˜épq'?×kÛYÇ5x?·,ÊU§ù?¼¶!ºÞZ?¤4R'*J?à³NÊiy?¸Î=?o?ÖT¹^õ•?ÀúÔ¨Êu?˜7+Ž™ÎW?šçÇFrwŽ?äéôG\'?Á%]šî`ú?Քsb€Ü<?ÍáÚ'J¿
?©Ðѯ®°Œ?«"L	Ö´?㘹3V³Z?Î^‹l–gq?çÂyì?Ña"óLñÔ?©mY	[ža?®hôñâ?Íe¡F®‡Š?Í÷"%¿]?ã4Ê
jò?·°PX´¬W?¶x [ÇÕV?¡x[$v©k?ÓøCÔÒ;?¶}ÆÜ??àq«…n-I?¿†Wٖñ?‡dœ/ø x?yNGŠOô
?Þa"öW
?¿V§NMIXED3FGL J1741.9-2054@¨u€4ì@˜ F†øÀ6Û¸KgÝÀ:˜ùN59@	ÈWQölÙ@°5<wÕ?ü&µü¦¯,¿Ñ½Zý/HË¿ã:*k¹b¿í2äÝÿhð¿ïwÅiÆPSRPSR?hãSS9û?™™{õ@t¿?î"r´}?¾º}>ïÿØ?­O©æŒÊ%?¾&l.'à?8| Ü÷@Ú?Z7ºƒØgå?ì(áë9kÔ?¾«;œRv?¾ tƒy`ƒ?¾ªãÔ.?Žo…Ûn?†´‡HÚ?êAYyn?¯FAgZV?Å¡½ªp?­ëµ5Ðs*?3ôµHÜ?4^˜•g¾?ï~BÏn£Þ?‡`‡8ÊË?Ï«|ږñ?‡NeÍ¡?S#Ɓ-H?_¡Öv¾&-?î}.î™À?ÂÒ{Ú¹@ö?®/ߌ…?ÂÓ0˜h?P	Ɂ…?e-ìZ?ìUøQ'K?³Yeu³\û?»µ+ägüœ?³`…Ì&A…?™5;Áº.–?"¾NÓÏTÏ?궖òö,B?­OÎÿ"æ¦?Áþü»¹g?«`˺ܒñ?E-ßK?ã?<w1fˆ?ï|àâó«?}_ª€3Ñp?wtU½KÐ?|¢´ðjXPSR3FGL J1742.2+5947@V àè@?Ï¡àø0À9õ@UZ¥hÀ;ë½¼Ž'(¿Ç®ö£
@ÕáWHfK@hÆÿ®K'¿êН<¿ämtkH¾¿Ütû'毿áZ3RÆTAGNbll?ïù¼Ž³ƒó?H§•NþÍ?/Æ;m~2?-"E»h`u?A5»OüU?D	'ûÊÏ?ï¦Ñ»k?ŠÝ»Õ‡i?rœt;Mu_?'<­"5¼?z^Ôõœñ?€úI.šž?ïcCàeÂ
?ۑy"
@?\Q-ÿˇ?w±lÒAÒò?‡€ßBÙ	?t1ŸLÈmà?ï®oÕX•?y¬a3˜?PK©†›æ?Khyû7	?'V®ðfW"?xIþQÛ9)?ïýmâí±°?2Q´t±˜Â?!¦M
?&îÑY®4Í?'{Óù"Ïû?&#Y6xÒ?ïàž'ÙÛö?iU"Oaué?[*O%±?T7?6í—?aÙgÞã/"?d3§"aK¼?ï¹
2"?tè\Þý?pqâ<=ýu?sN?‡Ïß?s–;ßâ?]ѹ˲(X?ïñÓa2í5?S™KwÃø?9©ë´#?&ÑÍ$¨#?V=GˆÓ—?R¬‹
5¯ÒAGN3FGL J1743.9+1934@EêG@0q¸@7Wà0VàÀ9ŽÊƒ*ÂÀ;Z´Î©Eß?ÜýÐö…¶@
(w¹õڍ?ünJ 	µ¶¿à'󆹱׿ÐláÈ¿]¿ÍíÖèY›'¿á"'¶®"AGNbll?ï¼J;Àþì?yz}†}Üô?pÞ:pÝ?p ·÷5&?q½âPØ6?lWª¨ú?î×9:'ÔÝ?¥äåoIÔ?ÈŽýi?‹·Ì50?"PJ¬\Ðø?¢4)"D?Î?íâ»ü¸?˜õH¢ùB5?™<Aoy"?ˆÿæj¡ý?¥A"´ô?'§K?
Û?ëoœzA'?ªAXôd ¦?œeÖ`®ÈS?"(¬è?½i¦•^)4?§á Ç6?ïâšwm¨X?gø"(?[_-+'k?^FÔ^ì;?_kã§$‰²?XdPðÞþì?ï‹øÒí¬?ž?èÊl?zšé¦G3?xM§OP$z?Ùp¶?‰Ã	)Ÿ`®?ïZO=¢?†Q€gъ?Š…•ìëð?¨JÍ[Ðz?Ž#âÆ#ßZ?yäÁ+ø
!?îµ$h?¤ÆÌÂ5Ñ?—iupŒ³l?€½äFM¹?¢_óUDÊ?‰Zb¼ÑAGN3FGL J1744.3-0353@5"?·¥ô@*
N wmÀ9œ}¬ðÀ;ŸÑß[¿Éw"\‡{›@
>µÿUá@'WÀ0\>?å#Û´ÇŠ¿åcÊøÒæ¿â݇®úBÁ¿æJ~É0õAGNfsrq?ìcÞF)?¸+¦Wü ?£¥¹ooF?¥8:cf?³¼T`}º?³
Y– ?í,?ýr?Á¸øjƃ™?˜­Ã:?¢[Y!lR?±œÚv¡?½<ï¹O±2?궂¿}j?¨Ëßìo6?¬Ùe09Û?—b
º'Ã?»ß=#R@?¤6šz"e?ã}Žt?¶"»ˆy-?¢µ¿õ"?–$ÏyA¸Ç?Ö­€0¼áG?µÚT¦ž°r?ïJE)ïq?Ÿh+'žáT?яÿbÞ^?†Ærë"ô?…íàd?—óY×ÌU?îøɍۨæ?®K‰(MË?ˆ}·™gx=?š(µ?"§òp÷ï"?£€ ¶YÈè?î\ø8¶Tæ?"‰7æe?•±FÀuÿË?†Ã!#ýee?ž¯²*w1l?Œt¡¦…9?ꈹФP_?¥·ÎÄ
ëÈ?Ã'Z¿'r?{ÐZ¯N»¾?ÃĨpÌñ¶?¥'à̧»AGN3FGL J1744.5-1133@-¦C?ñC@"^C ÚxÀ7ö›ÅÃÄÀ:Ùxà¼mÚ@.Ħ7¸@Øâ'q	@'¨ëF4˜¿ÙÉñÛÏôõ¿àÚz5Œe¿ê£Ö0Ωò¿ìÀ"•W¿PSRPSR?p}Y"vÂ?qѨvz´h?盧èO?Œó¢¥ø
?}s —ÒՇ?†d*‰ÜÜ;?u¿¿rsž?;¸Xçà?찛
Td(?¶n¸Ñ_‡?¹6£("F?¶jŒ´8>?«pEø?ûd¹á?ëøý_ð3?©o
ãL?¹h0Ž9Õi?£zÜ-&¤'?‡ÿjzì?{âwU5_]?í2¡´9r?¤	Š¶Zx$?³k­²ïñ?¡øB#>ˆ!?sü¢þ?vã­ð?ïšì¾ÀÖ±?‡ÿ™žd>?~Œ¼?€I§.#Ê ?"Ù_œ¨š?›M—]2?ìD5@îL?µoOèýXQ?»DZbw?µO¨üygê?·æú÷»=?¢-ÌÍë´-?ê2zqh֌?©à™`HF?¶…1èy^b?¢,i9†\Ç?œD¯ú‡"¿?"N¶†aEý?ìä¬ÀþZ?‹õ!-?±Én…ùü?–ù`¬ýŸ_PSR3FGL J1744.9-1725@#×Àâ¯@^á¿Î¼À8Å]Ó6À:ä9]ßË¿³»ëñ-¾Ð@9òj@›Ä?àj¹¿éùrû¨µõ¿á
ąšM
¿âÛ¼…¿×yµAڄµAGNbcu?îˆxŠˆã?¤õ³{ä?w•SHT=?q)Á5e ?¤…Õ*_B?¤ajçj$?ípMí–s?ºÆhY° q?ƒƒ²–Y?Š2:ï‡?²
 3š÷?¸½?©Ë;?ê6v€öò?®Æz?¡™?¨]~šÁ‹?˜Kq=fD?Á^p?©['ë,?êhڒT?¬I•<?tHN*´Ï?rÞÞ{™?źU"tvþ?¬.Ǭ'î?§)º?ˆüar?Xì
€®Rš?S_)¾7Ü,?‡t"†È!;?†ø핃Û"?ï[oz¿ÂV?–"8¬GZØ?oºB3¾·Î?qö+óÙ6?šÈ\"oR?'oH§'ƒ?î;˜Ë$|?˜@SÆëP4?"Ö~Ðð'?ˆõ`ž?¢[q‹u£ø?'32t€â<?íè"m¶g?'T1à?f¨æ>g³?Uy=Î(¬Æ?°L@å?'%'VÜAGN3FGL J1745.1-3011@vmú WŽ\¿â…'€ã"À73	~.IÀ9ºrW5q@æ|®§GØ@[Yèÿˆ?üÂHÊt,ù¿âáê ó*/¿ã"±_ÞâÏ¿í@øM"Q¿åȀl¡êOTHERspp?pku¼ìF?"®élnŒ?Í|)Nþý?Îöœ©ïR3?è€ÑÚÜ8?Ïu
s0#?'µ¯û^ô?"¸§]?Ղ¢±	;­?ÇÄ)®©?äö—аuî?ÇÇ°:<^M?±Ë-U"´? zïTIú?ÓÅp`ÿãê?µ©D}	?ããâ$ø²Ú?µÖç–/_r?"<Èδ…8?—~} ¡'
?Ò:,e}w?řmš[-?æI†"¦?Ų*E_ö?iªZ«E1?dU¨E´?Ñý'î üÇ?ÓL!…z—?æçŒx–6/?ÓJŒøÊú?Š¢Å"øí?•ØŸÓjVÓ?ؽ{9öá?ÆAFØgÆÊ?ã‹.?®l?Æ|Z†*ÉO?¸ŽIqàƒh?¦Z< <—}?ԼӘÌr½?´šâ"Á4í?âÍ4zå?µ[*hÌW?ÃÁ}s?"qOE
x?Öú9á'ï›?ÀŒÛ²» ?äñŽ‰V?ÁlûÔªÅDOTHER3FGL J1745.4-0754@2%ƒÀ€æ@%¦<OšÀ9ÿ}úâÀ;׎Ǯ€¿éòzv=Éå@õwæÁk?þ±Ø³iy¿é¢Å¿^ǃ¿Òïò¥¾.é¿×B5Ñëg¿át¨üì'ÓAGNbll?îQ¸5Øl?°:¤ÌÀœð?pb†ä´?pTá#‰¡?¨á™šgÂ(?¯ÿfÿÂd?ë£?©ú
–¤CW?ÑÔàã?€1±úø§ò?£¶ŒPäR?§•´D±.
?ì="ùà'c?¥®ƒ¦1:\?¡:{€éo?z†cCâ§?µvÏs¨ë²?¢'1>³¼R?ìsæފ©+?¨;VïÛ,§?e‰êWª¿d?aCÉnΈÇ?»´y·Úñ?¨ýêŒû?ï¼xÛwÏ?¥•*ÿT?bH«q³£'?_c­ü^!?šŸ[sšá«?¥2…(ã?ï'p×ÞÀ?‹Ñ"»Ïv?iZΆäH?gÓczZÝo?…
IßTã?‡‰)¨ÓšÞ?î'K?'Ÿ¹»šlË?'e)Ìî_ã?ƒJA²z?QuÌ1‡½?ŠYÿޗÜ?îºß(çLL?`ÎeÂì=?T"«\wí¨?G~E|Í5F?£­èeƒN?ŒîYí®°AGN3FGL J1745.5+1017@Alú€d>n@3BࡕçÀ9F–µ¹‹À;=4Ä,ë?øtþÂhDã@'žEzÞn?ý©ò!vr¿æњì¢L"¿×•&'¿âDîôàt¿î¶9ÀãWPSRPSR?±@«6?²f.DLeR?í0ê'?xÖ?¶ ëq5sì?"àÀY™F?šê¨Më?·›BÞÜJÂ?¾KY<(Ǘ?é;eÂZ5´?Ç\ÿ·}&¿?¾‰¿û?À`ìgOx?ËÒµçŒ?²Î†Ï"2?ånî}K°-?µõ«FüO?¼ã!ô'¯ƒ?¦o©:‰YT?ÄÛ¢Í
Ô?®Èâc`BM?åºÉÒ*Û?¹ô0 Ö¦?Ä98÷©€~?¬TûGôW?¿j±NÂ?¼âÚ!/?ë•ý~¡f?¿˜a ®áª?þ¥hØý?'fûðMpÑ?ËXÌÌï(å?Ä9oÚ¥Ë?åh0­
Ô^?ǧc?¾àýËE?º¡,ØG¢?ÛqÔX|Õ?³Lןé³Æ?Þïc9Th?³¨"φè?¶{##'ù? p6dd/_?ÐéY얧Þ?¬8-…??䞦Ñ]?±çB%s¿Ü?·j_'î¢?&ÌÃH±ÎPSR3FGL J1745.6-2859c@vJ r~¿¤¾¿À`2À6	škP°òÀ8f€®I#?Ñ1뷕ûL@ä•Wëy`@'þ Œ=¿ç¥ìù'þu¿åõÁF†Í¿ß%áË·y¿åß äçuÅOTHERspp ?'ù+4)™?¢?¥'²`?¦0BýrŸ?ºÀ¾ —Ã?î2"ëi?À8HàˆZF?»ê%^oˆ4?Âήïl4?´ŽÛïÐ>?±Q´•?å?éðßÖaBˆ?ÅH»½}Eó?º@¸	¤Í?¦I膅£j?Á';£o0d?¬iEzÜ?ènïšF?²'=áª? …ôו?°B,U‹‡9?c'I^¬Rk?gßÉR Œ?îì5Wr$,?°ÌÆ.'ý??EÍ(?¥HÕKÚ?¯¿Æi9?ā>»Éç?íƒl».·?Æ.'Xÿ?Æwºêª¶Ö?Ƚj™¦Ú ?¾Øæ¿?·8>Ð7+?æžÎ'¥Ò?ÊÙãßk"€?ÁŽš.!?«…ðaªÔ?Áë©Âí·?ªâÅMog?ç!qh¼Æ´?±ØÆ»ßÁP?–ØZ…õ?¯5‰Û¨¶,?eft~" Ö?fÿp_Låa?ï3Ö·×W?°"šsǝOTHER3FGL J1745.7+3952@Pd™àvp@=	› æÀ:¨KAFò-À;Õ«ïÝs
?áû=ЕÉ@
= åRՐ?ú÷x_7H¿æ£…µOòJ¿ë‰IáZ¿Ú)ҝ'n?Պ`·áêQAGNbll?ïä4ÕÊ¢P?hÏI
þW?1pæÓÙ@?0÷¤7Š¯Œ?i
›4Öw?hN~ü©ñ?ﯙl'èd?'°áÆñKö?qçžÔ{˳?sF¢ÖÎ@?vKªèb7?z'f;²z?îԜ0ðW?‰mèßԛ¶?"i6WÑQ?rvé>¾?›7Þ֟y?†]iQM0¨?ïkl‹ª©È?t«ë¯$Á?M8.^'?fw‡ÿö…?'©´ÄÃ>?îONRæ…?ïöÇHéî?MG´'ª­?&]¿öL¡û?$bd;Ȋ?OLŽƒ'µ?K2EtÕVÓ?ïßÜÃ~´*?qÀO9›Ñ†?\ŠïË?cvDqËQ©?aÝĬÅØÖ?fTúÓý4ø?ïiDÄ¢~<?yŒ†öÓ«>?x±Ónžæ'?e"ŸTzÙ?‰Uå1ÅÄ?vjڕ?ïé`Ç'Ú?bè7@Æà?BZl£m:ò?SzNªÑÞ?b"eVS?]àÝßôcÁAGN3FGL J1746.3-2851c?à ÖdP¿ºh~À5 ÝÀ6‡7`ÆÀ8·*´ßp=@áhy@-5ŠÑTÇ?óËá'LË
?í}Â"¤Å¿Õ¿Ó?,» ¿äè‰÷e&Ë¿êO© ø³…OTHERpwn0?3@VRW?3
N*8'?è±d	¦D?ÍUì.¡o?Í0ϯïá?ÍS¦Ì™1{?YÁÝTTå?y[‡ë ?à:/°")?Äv'ÏL?ßr%ÃUù?Ä&ÊÖ8Âz?‰Ç£¢nðÈ?‡6Xïeû?䍶ϊlU?º";+­¶e?ÖUC ¶?ºg˞×û?n$oQ˜¸A?yBº±·ˆ›?Ænì¦öá?¾ZÀ€c<»?êF ‹:Ü?¿GËcɱ˜?#ú[Yð™?','?®•:?考sâ·?ÏÝBy)ë?Íøõ<áƒ?ÏÜL©sMÍ?T½
œÄüß?q%4Í|?äsý›KË[?¾ègaQîN?×G¾ì Ž?¾û/e8?"F•¶l*y?'b'0e[K?âþŠ†é­?¶Î"ý¯l
?Ø΂yÂc½?¶ãÉó¼k?d+'":0ã?}Žÿ«Rô?ÆÆc^¬\?¹퀌Ýh?ê:<k˜ˆ?ºGmE MIXED3FGL J1746.8-3240@vO¿Î·‰ÀH?Z³ÖÀ7a<ðKWÀ:0ñ>œ@×Þ§À£Ê@ú§S@™Î@o$¥ü©¿ß}wŸžÁL¿âL2_Æ«¿è™»L
´S¿í<ôàg3kPSRPSR?7\Ð fݵ?<è<·l£T?îܦV–d±?§B"ÂGÍD?¢àôö‡?§H™»—4?8ø–<xâÉ?YCQP7†?é=ÖOW?¹8 uð?Êü*w;º…?¹6]ÞM@?"GB<n"ü?‰6T;EÅ?çØîW¥È?µOÉ\xþy?Î^Zíü?´\)h£?}AÕV??q·†§j
â?éù¶ÿtÚ?«›–™Àù?ÊÖ¶
­G?«=:!}Âè?,3;Oñ?/á,ƒSJ˜?î2~Ü õ?±Gß~rz0?¬»ëô›?±B1E9?G''–š?^­@BúÌF?é[½z/"?³= ®½š?Êyäl"ü?³2•ÜUs?¢{u<ÿ ?™²'OW²î?èZú"}\?³"‰"p	?Éõ8]¶áË?±iߓ¬x?…ï"ÎfHí?x+]ŒZ9Z?éjeÆЬ?¤»Ä˜Ÿn?È£d;Ç_?¤ˆ/™2±ýPSR3FGL J1747.1+0139@:õ€`°@.FÓÀ9n‡Êd<ÀÀ;©¿Š¯¿àl
‰_©x@Ò[]@%ù?œx¿å]yfâüÔ¿çv4ËÊÕ¿èŠW+±¿ïþ÷'ò[RAGNbcu?쏠[w"?º×â,½? |G»PZ?œ¥Jâ-Zw?³D¶'!q¯?¹79¥ƒ«È?êü]ï§ö²?ÅâÕÖÇß?²fþ¢º?´PœÙø«ä?µ¶røt8?½ø:R¦ú?è;Ärõ"?®ÜŒ©'Ì?¼F1ßî_?¢GcΨçb?ÀíÕIâ»æ?¥+E/ã\+?àú=Ûz1?¼x5ú@?¿bÇÛ?´o=œ»?ÖJëÁY§?»°t§qÉq?íƵ'¶ö?µ§'i`?›c§/´m?šÛ:á˜ÚÚ?¦ÂÛ¤"n?´‰õ¤SÔ5?UÁÜ?±Ã}sTRÁ?"Ÿ¥u©? ³=¢«n·?•®ÐH¾pû?¦@@ۈ?ë¾Wâü\?£»E÷í6?²E.Çs;?š'vEê`€?¯%³‹
Ê?˜,yíSk?é)by>R?®W!Ê·%? 8{Êó?""Õ'÷œ?Ç4HWÃÇ|?¬ Pf ¥¥AGN3FGL J1747.2-2958@vt´ ½¿ë@~ D¹À6rA&:ý,À9gåëoO@¾o›Cgß@bqŕ 
@yV-3??ÄéVäEíԿ丄&~Ÿ¿ç*‡ÿs,¿íœ‰8#PSRPSR?Fo†\¡åT?I6¿?åS"4
?Ð-¤#Çk ?ÕM¡Ô%±•?Ð)ð«ñ'[?5¬H*?`ÕÄ.òš?æw¼âÉä:?½Œ¥wp?Ó"ù)L*?½‹G(U/?']g'¹À?‹#´­I¹W?äˆ<ýŒ]F?»^—î|S?ÕÙ´ž¥˜?ºÚoˆà ?iJNäYÓP?g £>)¥?àTà
Rz‡?¼XDÃ1 <?ß#«NU?¼|á¬F´3?1Gq¶Ø?4} Þ`Vþ?ä®Yh7] ?ÒÈÏ	ƅé?֞ûRò\?ÒÇФÕN?A:ú2qö—?eÝ®­æ_?è5¤á)?´·
Ÿ…?Ï1~l|?´
)€€8¸?•NßL†_c?''	l
?äã›(÷c?·CîüO?ÔãÛ¹œã?¶¾~ œv¦?j5˜rë?j˜€Úv?áµ9y.¦B?¶å›(N¤?Üa!Ý9E`?¶ÙâÄ϶PSR3FGL J1747.6-4037@uâî_ú;›À˜Ü )€­À8Ü4mÅÖ9À;8>4îõ?ð{"§;™@¶ÇÖÃƔ@•¡ŸÍeN¿¨—ÌöúY¿äìȜÄû¿äâCåe¨"¿ì
tñÅÄPSRPSR?Ҍ­œt¯?Ä¢•È	?ÝX²4?ʔt9Y?ÐCE'ž´?ÇÎÀL¶½?Ŭ\/çà`?°;´çS?×ß¼µõ½(?Ày;öPSÕ?ÝJ2R¨?Ãó:}ªP?Þ@ˆdº?¸'ˆ6ÓxN?Óéï'©?µ®EYB¿Ø?Ë­›3¡:?³WË@ó ?Ï‹¦'Ï¡?¤Va/¡¬ƒ?ØòØO6õ?«hò`CÝ\?ØgÇTgá;?¨i¬˜¯!?àzmÀ‰?ÉB¢yg?ÒÚ7¿ÝÀ?ŪWþÞn?ÊbØ£€ß?Å7ºÞI?Ø	úvž?ÊQíâµÜ	?ÓÆæ?~_?¼ôiýRY?Ô/î]CÂ?Ã.иi¾`?ç\rƒnù¢?°"(U.'«?ÆÐòìq,é?ªÿ̾'?·z†¤0¥? yØ;í¸?Ý@ÖWm­¶?£ï×
Ïh·?Ót¹@å¿?£äZ!Ór*?ΔàÏZ"?žCI-ÌèMIXED3FGL J1748.0-2447@¡v m³¸?û€à»AÀ7VãÉW,À:$GŠLá@ö‡`±ñ@JÁ"àL[?øQO¶ñï¿Í¤‰øóB¿ÞY bvÞ¿äðè géô¿í( 2:OTHERglc?›´¿%D]?¥Ñcb	'M?èÃIñ¦?Ë=;-í<ô?É|FAؽq?ÊT9p"?|.¥1Ð?ŠEÖ1Մ?å÷ë51~í?ÃðÈ'(ˆ?ӟq+Þ¢…?ÃÇÓÇEó?¥¯.kÎ/M?8µÆ?æ(šõu?¼òljG­¥?ÐøäG½®Í?º˜OË"l?œd%8=?ŽíÞ+?ã×Úµ?º
äQFJ?Øš
¥ó?ºÜq/˜?š+j8™SÃ?¤jÁ¿Ój ?èg'ÁCŠL?Î{]P_‹M?ˇµ–zU?ÍGú.sŸ¤?‹œªXHA?•
—_'?èO!âd?¼Øª{" ?ÎøÑs¶Â?¼æÓYêé)?¦³ÏsäM?ì:6?æ·Ùö$+?·¦Øƒz£~?Ïs¥ã˜¯þ?¶f6–š)Å? ¯b´kí?'7²ã†f{?åtiÌwgk?±žÛü)V?Ó@u¶n?±¤xuíðPSR3FGL J1748.0+3405@M¬BŸ·ÀÌ@;.¦ÿ³©æÀ9œV÷]šÀ;É,¨Õv¿À(UR—Òo@†íð]÷@²ÍOÔ¿æ]ìÎ꽿ã—B•¿ç‡@fn'¿ÚI-è½æwAGNfsrq?ïëÙËka?_xG–?ZZkÿÀ?X°+!Ýó€?L"¼"+?L*R€´"Ú?ï±´Î?ˆÝ؞ù;&?oŸ;Š"Ã÷?'ÿkÔé?wVZN-÷?{!Äu6J?ï™M^ˆ?†°0ê£y?…÷¶y\	?x\JSï?
?'û>ÀŠ?€=æ/÷£?ïؐ}™¼]?sÍ࣏V?
bû¡ðw?Ò·ú"­?sƒ²'kÑ?sž2êêÃ?ïø³šn"??J×YÍö,þ?Br+ãÄ^?B~À¸áð5?6.I?~¢?9©îl›T`?ïä
)Íó'?hglŠg®'?Wx‡ÿ$ý'?T Ûâ?`6'l3nê?b'ÔøÙ? s±?m­yܳd?tw,Ü%á?bùøœ6ì?y¯ƒ*_Vª?dYͧÄN×?ïú)¼3nå?IÞe´Ã&>ÃãÌУåé>ӏÆas¤?GE,#6%2?IØóTvÌAGN3FGL J1748.6+7005@Y!ˆ M@>µ 6×-À7͙ȓ'(À;#Ö~ý6!¿²µ¹¶'à@õ΋"Çs@ƒäŸÒBØ¿àtæu¯¿á'À¦<¯¿àr|Ý~ÔO¿áªÀÐë‹AGNbll?ïþBÀfYs?&ŸŒŒˆä·?
iòÿ—5?(Övn¹?%9y½–?&	#2MVp?ï¹I]þ:?‡Ä>n¯×?o3ŽÀª,?'$'ÔxÃ+?sÁ‰'_=@?vªïé³?ï:4¸ÞD?'&i#Ħ?{šŠ	¢¤?z¬'ôœ?'ø;¶½Ö?N«°Ô?ïûãG&s÷?N\;VÆÃ>ÀR¡Ákœ€>Ò@hüa*?@b'`œÕÏ?N	péjMÂ?ïþÞæ»òp?$µ \—g?¿™9(PT?æ·e$%?ÃdUoڅ?"øXäX¾?ïç"à™w$?gwc€<'?UÐ]—ä!?T^ î]Æ?[ê,}8DR?aœð"ÃŽØ?ïSqÔPC?Ž¦Jógm?zz"môã?'ÌÂüÂp?Žͯñ€Ó?ŒX³¸c:5?ïÿU-.?$'\BäyI>­¶øŒ¥íŽ>½Lú7?é:ðB?$‰èH>¸AAGN3FGL J1748.9-2021@÷ŒÕ£5@TRRá#À7éèEÏÀ:"vOèu ?ß²žDÆzñ@‰Õ®óò@aŸØ"¿ãÊc0Q¤¿é~ùÞ1¤¿äy–ÄÓH¿îmÁBá&OTHERglc?ØsžÖ¢í?ÇcrWئl?ÕøUoPÎW?Ë­4Ÿ!¡n?єºD¡?ÅÜ`=­`?ǕûÛ$¡?Ç»)‡ôç¯?ØdôˆŸî•?Ååܾ1~}?ÛÐKyr?ÊÀöΗ?ÔÿBžh¿?³~–¨Îk?Óú¬µ
?³õ4¢ñry?×éT£¬~4?µpråßy?Â誮Œ<?®¶äàMã?ÎËnÄ¿ô2?¹DlÊZ?ã"ä$_ä?¼£Fdà?â61Sç?Ìv'K¥"—?Ñú7ò"8Š?Ê5'G1[±?Ã2Ì ?P?ºäÔÊ
ç?×ö9€‡ØZ?Ѝ×h ¶?ÕÏË£ñ¦?ÅƝz)?Ò9úÚs Ù?ÄnDÿG–?ÞÉWnÉ-Ó?´Å*cxAÒ?ÑXèådÒ?±y1'Œ•X?Ͻ?P¢Ú¶?¯3.a¯uä?ÑÕ÷Æÿ?¶¿µ›¯}Ä?ÅáWWn•¤?­ŕˆÙQ?ᜮFd­?¸€s,óMIXED3FGL J1749.1+4322@Qi # –@=#ì_9K{À9
AðeXIÀ;¬ŽÁÏBÉ¿ùù"Œº8 @úVÆz@ù¬ƒ(¿â‡½m֔™¿åUifK
š¿Þ4
LùǛ¿è¨ú_­AGNbll?ïÁÔ灷?uÝ//•\Z?gq0Êó5Ç?e!%]íO?s\óë.•Ÿ?o8.ú"H:?ïx9L^?"í#oËÞÉ?|Ü7dJvT?Å#&?ƒƒ'?dF?Ýì|7?î^ž"e?žŒšô?'k6JŒ?"óßþ[NÖ?¥´h^r?˜	ÿ9.ëh?喙+½ý?™¾91"Ø?Xl.…6?f±y®C?šé1îuÐ"?˜ØCÕ@.†?ïð{zõ•?Y¤—×Þ?P	ÒBÔ?QXHcï…3?NÄ¥3W#?M3sDãÌ?ïÖn™Då?r«*v ó?aGÔê?[m¶F5‰ô?hJJÂj
?nJ¾àf	Ý?ïPà…f[Õ?…vë›yU?'\ìåÈÿ?y}(zæX?‰k@¹Û7Ý?|¶A×ÈÛ?ï×^Cµ¿ó?w`ˆ¥±M?(-² "A5??¤yw£³'?sp²Wô
?wB0¹:ZAGN3FGL J1750.2-3704@v^ FÇeÀ+_ª4œÀ8³¼Àæ½À:éÜF½S³?ï|@Lv@
hhîV	@³Öà¡ëοâÓíçпåjÑfe¿å¸ÜP'`¿ìˆ¡ú'+6OTHERglc?¬ÌT@š?¤­kº‰?â<$zw"5?ǯÞ2-'M?Ø5ôc?ǀÜWóö¡?©@¤-Bï™?°-»qA?àãÍ}Ýâ…?Á±M•_"O?ÛP~·Yã?ÂÕ Ù²l?Ô§Ïg[Ú?´XXŠ³??×Pë•d֙?µ&ëŸra÷?Ô¨l›3͍?µÑœZ@8?Ã|k¥.g
?¥ªubl?ÛÙg¤BÙ³?°´@|¤ø?Úhb‰%òÈ?°}ôU/î?Â?erÂâ‹?¸Õ9cì?ßАUE?Åo0±Æ?×¼ñvv?ĝ¬E:>7?ÅD‰:Š?Ãö\ÀAÆk?ÞIÆ}Rf)?¿'܁ºn•?×ôå«Ò?Á"Óæ``'?âÉÍV£ê?³)Ѻ¼7?Ï^±g°?­	VñÍd?Åz»²ô¦?¨:jl×Úø?ÓwD–g?§ýů™?Ø·ƒxß©?¨êPCÎÝ?ÓÑ]CÀ?¥§'R0MIXED3FGL J1751.5+0939@Avf H	"@1¦ý`OÀ7ù¢(´T0À;l5ç?úåÙ¡q@|Z
w¢@5÷Rñj¿Öp†Ҙ¿å=WÏ¿ã Áõ
¿èî>D´AGNbll?ïßòŠ\Ëï?i잩ã?W¯+Ÿ£ÿ?WºO¹Õ
?d5ߗI)?c¼Ö\.g?ïƒ}õ"l?òsÉ}i?w»'?tÈ
Yøn?ƒ—¤ýõì…?ŒVð¼;??랎½ac·?ªØ^ÓÚd
?¬‹æ‰ü?ŸZ"üú$?´Å–ÔِÉ?£ç"» 9ø?ƒ¬"À?Ÿ¡ap$® ?® þ"þO?'p勵?¢Ó¤´(1?ÐŸ¥?ïò½q2?VyO¸'5è?NŒnÉ1á5?MÖXR‹Ÿ?Fk»þߟ?Fú'o96î?ïǹ˜ùœË?©ÉÚ •?eøE™å¶R?`¡ŸQå	?q'§ w?{Tè>Dk?ëü—ÁÕÖ?©Û讵—?°<•z®¥x?¡¾Â, J?¯½c[»®?¢t1ý"p?ïRsݦ?õ¬"v?x•ä,Œ?nÌÇá,¡?€`›Y`ç?xDhÂ8­œAGN3FGL J1753.5-5010@udvâ—À'ù¶^À9Jûüe@ÌÀ;^&>?Ԁ‹"ò²S@9DM·ÃÑ@(Ððž¿ßk6cƒ ö¿ä뜋ýÈ¿éÊ°¤o¿ïÿÇo.¦AGNbcu?ï恚kÉ?f¹µÙ#?a…¡GirI?b´èî)2?P×¹Ü z?OFµ#h?ïd܏§A<?'(pÌwÐ?umžtË?€Î˜¾Ð"S?ŒC%@A¾°?ŠõÖ	÷?ìº{€)?¢m"|vÕ?±÷&àN×?žÞÀfÎEg? qš†…i?Ê	ÂÚ,G?ýÅé?‡2 x@d'?Y¾J[[}?]Ç}ûÖí?Œeµ1<Èd?†@s–-\?ïðêB ÛÐ?Z9[àãD‡?U è¤4ûO?V¸»v¤Ô?B#}5 ?<Ó´ÄwÉÊ?ïË:´d~¸?vÓݲ­!Æ?[ÖM|§Ü?\4KâX²?sm[Y
?qÿN€žÒe?îaLûӗå?–j†Çßñû?¢/ áÊPj?'™Mp*S?Žî=y¡ñF?üPg[b?ïä…0"æ?ee~éÐͽ?>Z…Úbs%?6¾·.â?g¯"y‡º?d®Ú'DÎÉAGN3FGL J1754.1+3212@LÞß¿î—ù@9j´M,ÙÀ7ôkõ oÀ:áNÊϝ?êÆ"Ì¿@Ú¾[?þl>ÙÚ¿Ýö?ý›÷˜¿Ü3
Ú¼¿ÚþE(‰Ñ¿Ýï¯f"AGNbll?ïý‰ñ"œ?*†Ê¡?ù ˆœ¯Ø?êìj9B?*òn–™8m?$*·)hφ?↑æÚ%a?|íf²}÷k?lÌB‡eľ?mq‹c?qÄkFû]?u"¦êˆ^?ïfå•?†aH¢ä¤?~	ìûô»?{Ë%—iî?‡AÉHêǸ?€îò±Ü?ïݸ2i'H?sí]þóA?,Íù{'? ·•°/›?påÿ?s¾øùå?ïþX
¶šå?!h<>¡¡?ÑQï'ì?_5õã",?!ËAÆ?™pÿ÷9?ïäJpý?hmöÐÆÊ\?Vå'Nš?Sé⨝jÏ?`C(ñ>?cfp§#ò+?«ý5?QKjK?yM­?v´˜)ØB®?€H­9=÷?v"
ÒÉ'?ïøÙ o̗?J®±Ôî|Ú?ú`öÃ?õsw‡j?K(
%6ª?J'Šµ‹eAGN3FGL J1754.3-6424@t'ñ@ìFÀ2r?©c;À9Îw/†FÀ;­±¨"(?Óº0q.@[¹ïÐ\ú@«r`o¬`¿åø¬˜5&º¿äâƒ3ëXÿ蚓Ð4"ä¿á£¯ƒAGNbll?ïÚ¼~߸?lÔd۞º&?`_?Ê~'?aˆJpu`»?d䦭Pé?a¤——sh?îÃÍ 9úU?¦†úÀ
¸?">n5¡Ò??‰gÉsïˆ?gãÇ".?¢ì8Iˆå5?îtÉ~''?A²c%O?".¬ð÷?
?æBUß?žM¹ßCε?‡.ô$Θ3?íÏ¡U?™ÆÖú,?‰nŸ'ʊ­?¬q®09
?¬ªG¿Úä?˜^l7"ÓC?ïòËÍc?U>(‡?D¼‰(ÍE?C='…Á?PZ'
tGŸ?M…sŒé_?Í2£@?ŒQì—ÿvÔ?gW´Êˆ?dU«+v(?ƒŸ‹[øS?‰õBÑz ?ït´ó<M8?rj'³®®?¬oFv<`?e¢¸à/wá?'ü‹M¼?gåŠ*]C?ïƒZü·x?y†Éè?p.¬Þe%?]îê¬xBÙ?‡êjç[?uP4ó•AGN3FGL J1756.3+5523@TßÞÛgš@=·™€o&)À:M‡rO©À;áËÜñ?Þ[ǤÍ\ó@o»îƒ*í?ÿ°ð`$ØÒ¿Ø/óÃ[´Ý¿ìn`mŠ?¢A>lTð{¿Ï÷Xš¼ýAGNbll?ïà¹ÞUÜ?lÜ<Á¦M?@'Êä†z??͉ÿ.8÷?kB}eŸÙ²?j¢-"ÐT?ï‰*5³–?ŽrA_¥e?yÝ-öèê?'Ù՞(†É?€Æ۔æT|?†)íñè+?î­«2âð?Œò"ª9Èû?Š›¥Âo?€sgÂc<½?ËÏ[NY?‡7Íælü?î®hbî6?œáÃq1Û?rÚ¨"™?†Š"n¡?¢Ç^Œõ®?šL•?ïòÁ×.O?Yr·K<³?,ýI®A"9?-¥¨xŠô?Vܨz(?Wœ"!æ™L?ïÖ¼7±Ð¦?qŸ»ux.e?c4l'Ð?`Ù՛ÀÌÍ?f3"+Är—?i€P4-Sª?ïUóÉT·?€•ÑÀ~ï?€W<2Nq~?wÑ¢ryÐÂ?Š+чJ Z?um£ãē?ï¶ææ ÕÅ?x"GµŠì?i¢1'Ò³?gîû/gŸí?w»sÏ~¯"?r—-HAGN3FGL J1756.9+7032@Y?'à°«@=ûßä׆À:Á#å¸VÀ;üˆµENJ¿äó|îí@§†³bîb?ûIÇÚñS¿í8~_\¿æ´
ýÁ§¿ÒÈ ukg¿É…\¾ÐhkAGNbll?ï÷÷Gl«?I]9•1?ÿÊãpp!?6ÌŽj?L"éÇSðÿ?GÓÛÉS,Ô?ï¶ò+<U?¹Z{_ëx?m»Â‡¾å?n鴚¾?u©	W!cû?|uKauaf?ï(ª\ú?"¥s[[4H?'eVˆ°7Ë?ǹZ'?•è?k'"Ç?€á™;ã?ﳉá&`?|Y¶1¯?h?&…}$SÄÙ?0¿=ʁ­~?'Ãqº›‡†?|(?–Æ9?ïûÛ|¬½¨?5	Po†Ü
?Uš	q(]?‡2D^
?:N´•Ÿ|?3 õ ØÐ?ïä¬é¾±?dë4Y_€?Xy7œ?Th˜ÀäµÄ?_o•/ð½?^k&N$NŠ?ï†%®¨?nûôÂ/?v<8gh?ZÚˆ@ ?ƒpš.+lÙ?g¥šÜuCq?ïôA'¾Öa?Q_Ùù•?0>t8I?¨©¤g@•?UùÖmÑéé?P:æQù]AGN3FGL J1757.1+1533@D–uŸ¿Mˆ@2ߏ`Z³«À:-LBα©À;ŸÙ0ˆ^?ðY— ñ@q•înr@\"Dž?嘖Ät†¿Ø·§.¶){¿Þ™À&Ä¿ïÿÞ&çJ|AGNbcu?ê:;ˆdp?ÁŠ…ÛÝÈ?Ã0ü·¡'?ÀÓ¤™õ+ˆ?Ÿ0©>rïp?£|°V~ϯ?ÒGýÎ*#?Æï ¦=?â[ùì_Ô?Çç›~ºßÔ?Â]‹´²,k?¿³`Ñ7Pà?à–—Óé)?´bNEžŸÝ?Õ5ÖÐu'˜?²¯Sx)ß?Ã9ó–;§?°|EÀ#}%?ØÖV›9¤3?¾ˆ
n ¢•?ÞË2"¼î]?ÂRVw?À¼î"Úß?¬ÿljäÞ?ë0'¼Å1'?À†Àr/&?¾O–k;ã0?¾
òùP? W·a€£~?§K‡¿"?߅ÑYéM?È+ðdžoy?ÙW_úfŽ?ÅhMŠwh?¼Š…r'?¶Á)àI?ä©ð÷ö?°_pIôR¾?Ðvd`ýy?¬ÿRëf>C?º) µa?§UÓ}ˆD?䶗êþø)?°)¬¯rŠ;?Òíхª_¡?°¿Âüºx?­'õ#™gd?˜goÁVdMIXED3FGL J1757.4+6536@WÑÇ@0q¸@>?ÐàÀ: À
¡©À;þÀ°^×ý?Þ¦mV^u@¥'Ð&Ém@‰ãŸÍh¿é*š=¿ê[Ôþ…½«¿ëW°év?ãP0…•AGNbcu?R8 ?±R` {K?ˆñM/"µ]?±K¤öÈ]w?d!ز½?d¯—Íސ?ﯹÆW4<?ƒ•—¥zWÈ?qoêS²bö?vT
	‡?v³2˜×?z¥Ê€;÷?îKdÛ?•C+†"ú?—§×AgJß?ŒI_M !ç?žë¦+Î:
?‰Y"}>h?ï¯sú3ô_?†¶€³ƒK?Q=0·SÐú?qù…]9¦q?û[[Àx?ƒvOÁ¢	õ?ï!³D;i?õî†Ran?› €S!?ù6Ñèy?E"äSúš?AÕ%Œ
}x?ïß\$ Ï6?s.Væ®X?]E^i!îœ?dÄ	]?b,¶þj?eo]$°"ò?ï:_Zê˜v?"4\Mê¶Æ?ˆf—ð¢?€‰›1†w?‰
œ;4‰?v¸w["?ï÷Õ?]bÙ'ë?-àY:x°?H¶Œ¯ÄÎG?I3¸Ö¤Hä?Uê?ˆÝÝâAGN3FGL J1759.1-4822@u…|€"ÞÀ'ê"ßÎ1QÀ8þXÒ)- À;S&ìÓÓ?â×Hêæ¤u@×E¼wÀ@^%à9f(¿âö¬…ڿⶰdGŽp¿æ7ƞñƒw¿ærI@¾ÕAGNbcu?ïöè1W:ú?I¯@a–?@5\÷{L?@ÖÖjðXú?D*$}åd?;Z|ÍësN?ïbS÷p[Õ?'[Ýë:ó‡?sLä `Û?ñN€¦?ÅÁ;?Š–`'˜Þ?îÙ£t[>?‰¬¢"pé*?>ƍrW?€ÌbÁƒª?"ŒËnš3?~æþ¨BN? ?€D‡¬ü´±?GH­ÖUú@?O2Õÿ?…çôûáp?ãü'#?ïü‹[4Ñe?4ãmü·Ù_?(5æzZ73?*À»ÒGu"?/fþxò?&=iìº?ïÈ[ó_¢l?và'©Ò*?[Ç7Í|˜?YògÓÿ?tà> wúÐ?s%"'±•$?ï‹Â[[y?q¬ueóÿá?{φgòk?lü@1?~OsÞ©'?`*žÏºn ?ïêâqBž?^Å8²7Åö?86=^ã?2-ě(\?bÍ)ô…?\í»Vn%ìAGN3FGL J1800.5+7827@['~¡Æ@=×ÿ/öhÀ7[M-°<À;>*ðn'…?"­B@EOÐwÒ@È@3KÝ¿ãnÒ]Qâ¿ã¡Â¨0¶+¿áÁ	¾«Ýû¿ä×¼Öú<AGNbll?ïü€:îq?Rê]ƒ>E? …x<"?üÔ§ó?6·SäZâ?Rº=Ãö?ïÃØzÞv?{Ûï–,¨?j4ƒý¿u¯?lqnFu€?qdѨä>?s¸úŒÀn£?î'u2(""?™˜;Xm?Ï?'XgüÇW?~§6·¸m¹?£B'á>à?˜7í1e5‹?ïñ¿Ð1}ž?bÝÀvèh®>ýeÞW–ñE?"ç_LŒ?\
ȕ¹oã?bÒf2‰Ì?ïþéÙ3H¾?1
v…¢Q³?	ǗmŸ†?h``·¯%?áÏHnø?0Ÿë&qû?ïå¥/h½?d§²þÆÍ?VQ»˜ùµ?Rõu—l§Î?^°O.4v?\L^I)É?ï1;§©…S?'ç«ÙÜ?zóÿN{Ï^?~ÙÚ`β?"‹70aÕ?Ž¢½2µf?ïýÚ,B?9›6˜ãi>àìñcØ%à>è¹ÙæÃË?0§6»nh?9yŒêLŠAGN3FGL J1801.3-2326e@¬ÐDÑ¿ÐB OÅÀ5™þJZ"À9lžéd³@w¹ŸôR@mÁ̾Š?üßÎoU®¿ÑNŠ§ŽNã¿ãoNlt¿å;ÇÁË¿èÙRav½wOTHERSNR?–äªÜY?¥es,Š‡	?¿`£]+˜ú?ÃÉU>Jé]?ë'4n¾ñå?Äûe7M…U?b~šëa?ƒ~³¾W?ãbf£3\Š?Ǝ;{šïÊ?Ù¼7u¯?Æ¡êýJª.?·3$Böð?¦+$Ȗš?ÑQD‡)»¡?¸…(á?äpù3Õfò?¹'FÞRN?ƒÍb}ß?{Päh¨?Þ†c µ?ÁkþOj0?àªþx¿–?Ác"¶Õáì?­G×ã‰Û>?¶$<ØõæQ?³épFüù?Á¾¬âé?ë®Txõ™?Å9<`è¬?h¿Z)á_µ?z]tۍD£?çÑÅÓUÊ?»žÛš<y$?Ð,iÀc?»‹#†Ê¬?¶K…N-ì?¦ÛkDHc¯?Ô>±@ª?.?µü`ÇS?ã}îåË?¶ú•®Óh?€ZÏï•ôN?w¾¥!¥!?âb£@EY?¼@ß¼Ù?Ú·ãwšQŒ?¼\=ÿ¦$MIXED3FGL J1801.5+4403@Q»&ßÓ9Î@;þßnÀ9g½¨l›4À;ÍVØS錿ҐÑ4¡®w@¶6b½m@`M˜¿æ…$J?ÇÊ¿é¡[j'xœ¿ãéUͬW¿ïÿY,t°µAGNfsrq?ïüy–Ö?6díÜPF?õUI¨@?!î†h¶ä?45òÿ´$8?1Ò
u[™?ïXÌǀ?œ N½Èåò?½0©if
?†òæIÈ?öeOú	?–æ :EÏ?ï;A^'}8?ûãë?Š\LÃ8_©?w{Se\@?†Ó['‰j?tQ£±)"?î˜Y뮺=? Ì9Ç%?Œðí;ÍΏ?‰3§&"ö>?ž|KôØ×?—ø<'¨¯o?ïýù¬˜"¤?)½¢ÏÑÆË?¤‹ä®‰0?»tÃÜÙ?!'í(
.?ºA|­"f?ï¬é0kéÄ?~‰–¡''™?tÔ@(úù?n–}
ÔuT?t·'Ÿ`Î?u˜Ü
g0¹?ïmf
-Ð?uç¶Ãƒz?…ï+̀"q?n¿¶>¸óâ?}n¡ï	ªÒ?j¡¸	æj?ïÂÚÏ*0f?ug¨èë1?bÀƒ¥}ÞÁ?Xa)¹(w?u2V†úч?s§A‰u|´AGN3FGL J1802.6-3940@v`—ÌÀ ٍ0À7?ep!À:žT~ÝU±?ýaÛQÊÍï@ç%=§*@ñVe'V¿ß·w=ׯ‡¿ån~P›"¿äEdNM¿è ÑxFýYAGNfsrq?ï¨ÝšX?'§¤<"i²?a¤õêf´j?i-Ë@`èU?_[ú¹"p?€©M͞?îÞ¢á}B?©™½ÁA(i?~¾hEº¥?•€…üwÃ?œ¨´>¶t?£õf$öO??ì? =Z~?¨?¯Whi?¤"¼¸Ž™?˜Ö9ڂ?³Ä¡0ñøF?£9•€ã?ïÐb²8??…š'u\?#ؼb˜?4½žÜœÂG?w6'H'?…'6ù°=r?ïÉÙùc·=?{ޛ¯_?`®p~j?b¹1tú k?r»Ë.§\J?v-	ˆŽµ?fJj?COt­?gÂ;ÍÙ5À?lò=V£T?†áq?‰þmLsF?íӜŸ)ó¼?¡²2&I¿?°ñÐu?–·Áúk(‰?£î3äÔ·?™õ?ù
t?ïõ¡G7÷é?^Bpƒná"?!4mih»?#œuvË/C?R–㔋ÿ?]‰jT8ÜAGN3FGL J1803.1-2147@ U,î‡Þ?ÊÔ)`T18À7!DҗçéÀ9º[‡SZ@ªu
Iè@¥öy|Ä?ùÍBM­\ð?ïýǯ½®ˆ¿à*Cùb¿àÀfÂ#Gû¿ì¯–kÅSPSRPSR?T€C+€»Â?P¹Äñ¹®?Ü2Ê˞W!?όVQ½¯E?áÜZx5_¢?ϐF½1Vî?MÕ®"×WU?fJU°Sú?àÛ­Ëú?ÆYK	Ø`?Þ:Ïcï­?ÆbƓøšÜ?Š»ƒ6F\2?…''™Ü?âÄx´Ú?¿ӊ×	?Ù¡2~œ,
?¾žT¶²üd?ˆéüB=F?…#›n8 c?×Ápý\üI?¿¨Þž?㻟©…ö?À:8W¾?\?èbQqH?bª+ã{@?ލI1ÕÄ?Ñ|ª£µ¯Ø?àè™fÃÙ^?р¸OoÝf?]-mù¼Ð?pË7§Þ?4?åS!Ñ?¿ už<Ê?Õ<¨OÈrÔ?¿´ý£.mÒ?ùɱĜ?Ï‡Ò?âÓ¶±‹‹?¸qÖGçùŽ?ÙN²ÿàå!?·É;€ô,?‡ý{N&•?­š¹Ét²?Ý
â—?·Í¯å>?á?õ—?¸ô¿~1iMIXED3FGL J1804.1+0341@>Ô}`}ï@(h³Þ¿=˜À9í´ùqp†À;^èÅP׉¿Ô¹öP©»¦@Ò´WàçŒ@xÀ†‡¿ã' »Ä3C¿å¶ŠE"²û¿ß¿
º9¿æ›kFÜ«AGNfsrq?ïêí[…W?eƒª•Ò|?5ˆ²‹jf?1glTuÐÍ?ba'ItºP?d\KO°?îøë/ZÙ?¢ª-)ÊM?x-´ÿó3?t€W–þSi?šàⳇå?¡zýˆqL?îònWª˜?
¤ý-›L?ƒ´Ñ`ßC?uo‰""ÅD?—×ÌadX?Š\8µà?î×Æøa;?ŽñX³¥}`?VT{pyeÎ?RûƒÞå/Ç?¡Ðì¡f]%?Ž£Ÿ™ó8?ïúßØuÕù?F¥½èÑÊ?!"9fÖ?ô¾'|5Ý?@ُܓà?DɉMw?ï´3r Ô?¥{'"à?b{¾¤æ?Zܹ GF?|¨XÐ+÷?7)ÕÃî»?ï£ÜaÕ?s£-îd?p"-~À?_V°¹ºW?}ñ¬•s¿?nãù'Ë?ïµD6P¨?hÈR]¨¤:?IaemÒí?59"@E°?ê!éT-?hB"•ôØAGN3FGL J1805.6-2136e@!5\ ¿Êû@?W¦'À6O«ºbgÀ9yºZÚA*?ü>ÐJZÂ@ì}'%VÒ?ü³~'W0¿Ò"ŸÅÒ=¿áñëjFÆ¿âõѨԠ¿äóEšOTHERSNR?ˆÚ÷'¹ö?‹|î/vyÕ?rû£H€r?x{48Ÿ¹X?ïy­N
¿?'gˆOh?¡¿
äH?³g
'š?Æ¡t¶¿?ÁÕ]–.?é;²RøöK?ÃSC*Rm?½ÙÈL¤7?ªò+±?²90é´N? ˜À/`á?ê>ý¸?°lYžÆ˜ð?¥œ{
vè? xM=§S·?µèµ"ƅ^?§¹9ü]۔?ëéߓè™v?°q–q G¬?¢KxWVi?¬É‡
žû¹?~v.Œ°ª?"ä§.äŒ5?îž\Q
~?¯–¼à꒻?¶"€þ@ø?Ãõ"™LC?Ð6]•îzƒ?ƒ۬¹†õ?åAP?ǠŒ›Î}?Â>8ÊÌÂf?«Ö£ëUv?º(Ï'×À?£i+_ Ä=?è+WèÛ\n?°ÓxúÞÒ?¨Ê÷¸dõ?¨ÎbË?À!¡GZT?¨›5òŠ‰?êjè2Ñ0?´Ý~.OTHER3FGL J1805.9+0614@@­çÖyõ@)矾vÉÀ9ìŽÐè»@À;£ŸM7Á7?÷x&º©ß@
'ë¡?Ë¥Öé±4?Û¨¢þiŸM¿ÈÁV8¾.ò¿à«ñ«uÜ¿í-b
çPSRpsr?Â$ÍÆ-1£?Åù
CE¶)?âê«ô©Ïa?ÑßÒ>?ÑA2'ç¯?ÐD">i?ºä´#wm9?Â/Ûÿ‰|?æ0>êv4?ˬ'°
8?ÉÌ­ À2?Ɛy4tQ?É`aù‰??²š9£Kq?ä_)éPÍ?·FÎpáº?Å"ù"«ô?®¬•¤áY?Ñ>Cæu?Àñ	ö"®?áÌ2j'Í?Şê3ü?ÇÔR®‰Ñâ?ÁëgÜL?ÅEâU}¾z?ÆÐÓÞu'?â'Log†?Ò¥QÍkó?Ð:v¬bQ·?ÏÁá½°áE?ÒYËökµ?ÍóôՐ¦è?á•{*~ë?ÎÍBúŒ´À?ÄùªyCkm?Àˆ'`²iÂ?Õ8"!H‹E?µ¬U‹oF?áŒþª"<T?¶ãɦfW?¾µú&»ðJ?¨0™(o/Å?ÙW'%«,¶?½ÕzÎÛÎP?à6_ŸÅ$.?½fyFŠ?¸ðfjNDµ?±ÙùtwUŠPSR3FGL J1806.7+6949@Yñà'Œ7@=-SaÅÀ7÷Þ¡
§#À;Zë´ï`v?ð-3¢Câ-@^!p¾0@ßGŸ¦Îá¿Ý‰V)q,W¿äp¡1'GÝ¿ãOK Î}b¿äë]ö͞¦AGNbll?ïúâÙBjÍ?<µ²zA'?3€vð0ÿ?0®Î?¶?5ضB;¼?1#çÅZjj?ï|uüš?'m¥K³Å…?y¡WkàB‡?t'lû´y?"½)N(?ŽºÏ_©QÖ?ï'f|Ù?ô‹--%?"õÚŸDM?zm²ÔáÀ»?'aF(ôº?‡ÊjÆ5œ?ï´S%¹D?šÐ"m¯|?y'Ÿ>±?uÃÌ«dQI?˜%{`E%?™27°||V?ïýÚÅ͘é?"è­Y´Y`?$Zîwàa?×lE¼é?ñkÒ
Á£?º0ëâÔ?ï͔š£§1?t¡?f®3ÀSJ?]h(šíCr?k½2$¾Cÿ?pŸíNU+3?ï|¥Ðż?'YZ̾H?| ˆ‡Ê?uO4¹w²Í?'»MºY–?~½Þq?ïÇԌ×
á?xË$›ˆ¹¥?cǖ?dŸ]?U¬ºþÚD?r1îi"?vævøŽAGN3FGL J1807.5-4343@uÓÞ²gÇÀ&9@LzÀ9è6°–5aÀ;xcNƒñ'?ñ&>Þb ‡@î)#øÁ@ö<À$È·?Ñ$Š#¿ÔBÖÿ«œQ¿á~?kOÚ3¿ïÿÞý¦ßROTHERglc?Ãp©Ða&?Ââ«;,¦Ò?å›xìG]Ú?ÈâŽ9?Æ!r~Ö'r?ÃÌâ;žçŒ?°úµï3Ö¦?²Ó:"ôHR?æ®^$·è?Ãn³v˜?ÌÉ,‰Z?Á,
ÔBѦ?×o	e¤õ?¶qI­à<?ÞãÁBLx ?¶È©÷˜z?ÃZkl›ÅÕ?¬aWø~ED?ÈHv?¼j?°ŒS¥ù?äúËD®Ó	?¼éé#?ÃÌ\­ˆ—q?°"Þ%ّ(?Í ¢ÕœC?Éç›- 'E?ãu~Ûˆ?ÊÃ$"3ÿ?ÄZ!e·?Á﬉=?È8´û'†µ?"îÊM–Œ?ãpà`䂇?Ã6"‡S=?ÊɁFo.?ºô¹²¶¡?âþmwbô'?²K=¨µŸ?ԓ@¢e"Í?°ë›B©?µ¿'½¡? (±i®u?ÚB¸ñ<‡Š?­Åá'C?ß °>¡¦X?²ƒ!3û?ºr[@‡Hx?Ÿ8(DÇâMIXED3FGL J1807.8+6427@W†À
¡©@<ó?ÀàÀ:žQ>ÌÄÀ<èÙrÍ}¿õ"§èö@Dt¤@½_€C1X¿É¯…°꪿à*:ø4Á¿â0@ÔÓÎÁ¿Ø#hÖ¿PAGNbcu?ïú‹yÜ?Hkj4¹?>A¨9·Ô?GF\å˜?*Å!¸§Á? Àk'ð^Z?ï·1Ìož?‡}'Œeý«?nz«í¯Š?'¿|Æê?u)ÃçV¬?wXÞÏw?ï+àGö0@?¼$fšFp?«1>¢Ž?‹¯S*¤K?ƒ±ë¯lè×?r¡p!Øò:?ïêMòY×À?cyÕhۖS?4'Nå?ƒÇ¿‹â?e0hîúö¶?cN6U?ïý†Óß?3ÆûÈþ?'àòÁ¤ŠÄ?29šç0«?{õiÓ>]?"œ¤(z?ïä¶óò€'?d¸Xbøá¾?W¶äíMËc?T®î¶SÔ?^Û3\kÃJ?\­-BSò¦?ï–鸸:;?€8rQ?€W&Il7è?~ûa)ô?sÜÖú]Ì?cs/ @©?ïüèqK¥N?:‡v+:>è‹'½Ä2>äHDK¦'§?7ø°¹f?9ãnéÞ{¯AGN3FGL J1807.8-5011@uuIàâiÀ,?{@À:¦Ë±DÀ;xût€¿ìäkWšy@înKbª@X+Àx*´¿â%Ÿ¿èðj¿D,¿è ·§exï¿Ë†)žÎ¦…AGNfsrq?ïïͧà{£?[Äԑ'jô?AäHŽf?DÒJõíy?WÙ½ûh‹™?U(¢ú?ïôã¨l¬?gö}X?oî}Ùð?€ß'^ÛWR?ˆ@‹lwzõ?†8-
R¨ê?îøõQ·i?"‡µ6EEá?‡i9<},þ?uxÐÄN´#?•Id¼±æ[?~²"Í¿w?ïuÍzØÊm?"†p³?!ùé¤Â—=?)Wƒ'·<Ñ?'"\ւž¤?"mÑSN×?ïù.²šò_?Eý· 	š?0˜úg^?9œßªap?Bø·XxL?>j^Ď0?ïÑz
'9?sÿ'-7ü?W` M@¼:?W>ÔÌ…Ö?qjÒÉ€z?p'¾qô?ïÎ?Ð?hÆ|¯0¸7?tª‰æO('?Zï×KP?~þC\?aj+>ˆ?ïåñ;¢?Y¼NI–üK?šì¬X<>øªñ'Éń?iÄêҌv?Y¨+z{ŸõAGN3FGL J1808.0+4652@R'³`<Î@:'
4fÀ:ÄIqcÀ;ððÄXŠ¿¶C²"b¼Ÿ@¸Šh#Tï?û¤h_dêe¿ïyATõP?ïi†âðµ¿Û+ý¥Ãڜ¿Ó'ë=Œc·AGNbll?ïöùÁ¢w9?Y¯OT{S?7ʜcÄS#?D»€ó-?H3«[䩚?Pm1hy,d?ïx"fŠ+E?'´TÔð<&?|ѵõ×E?zðìàÌà?ƒvfèžý?w#ùÞ?ï³{[Ú¶?"":§ID<?ˆ5u0BbÝ?~U|ã›:?'ÖŠáÉ?xI«¸/§Ó?ïDm½?2'?¦ˆ«ºÍT?‡#=<Ž‹%?ˆ_o+zåÌ?‡ÁSlŘT?…x»6îI?ïû«P6Šg?4/†F…œ&?#éZŸ;¾?[­üâüÝ?8°Ò6"Áø?0D»4Ó?ï×'þFÂ?q"Júš{o?b«Ûµ¥Ã8?Y2¨¶"q?f-E4Bu?l!Ió\b:?ï{¹˜ù?zd9§å?~má¯-ç±?vrv&X"?' ¶$?cª(Q¹?ïÚ	æK=?cx¾Öˆ™?cõä¢ô7¨?T%q;ôþ:?b	CæSÅ?Zº<à¤AGN3FGL J1808.5-1952@$ê;¡–¾?£z"`h®<À7֓vié©À9´rcÊ«?ù¥)Gwý@¶ktBG"?ým¤ˆµñ"¿ä»?܎â¿Õܾ²Wց¿çíß¡»§¿é!& þ'ÃOTHERglc?b˜Jw½Ñ?a^ß¾Qîå?àÒ<¯ç?Ðm¥Ÿâ3?Þ6Vjá9?Ðjú$Hߘ?"1ñëó_/?Ï0¾ß…S?иfyí½ï?¿JÜmåÇ×?çSû¼?ÀJ¦àÄ?ª 	á…`?™òØeŒjÀ?ØLôIj}?¸'Ô±Ý-#?â9;ÚîðÛ?¸Š¸G ?£æ—•†° ?¢¤°é9o?Í ,÷–
T?¹ù±$ƒJ«?çY‹HëM¹?¿ Ö,®?c½mŸ
ù?j¿+Ñvt
?áµBck¤?Ñý:YSi›?ÜnùûA?Ñþ®×CsG?¦,ѤŠÕ?§ÑJ)©N?ÔU2ž°&E?¿:i™‡â?äè5J(†÷?Áb?mܯ÷?µx~CZ+?¡ñxsÊ?Ø@»gõˆ?´šö˜"K?á0ãZ,ò&?´ºýß)ËÊ?¥|±àÅúŒ?©5qÓN¡?к&]õ?µŽê"¤ï?æK)ÎÒØÍ?½ÎL(Í~£MIXED3FGL J1809.4+2040@G¬Ì W"ý@2:X@2õ÷À:2@ºˆ'À;¥:Ùâ)?ÜR!ñþpÅ@
·‰Ð£Æï?þ)¡-¿ä¨©¶—¿íõfß捜?ݜ—¡ƒ;¿ÆìàϟKFAGNbll?ïۑ–jåý?pâ«ÛY‹?+òp¤‹?+ƒ"ZÓ@i?qW¤¬,v?p»Þ²I3?j®l?Œڍ:ø?p´È<ÐÛò?'"U…·N?}ôX»Q&?ƒÖs 6?îo}ڟ"?'U!*Ù-¿?"ñe9h÷þ?u0;¶M|?£ËÕÂCû»?'~',íé?ï	³+èo?Ÿ|t¨pˆ?DjÌ#=?`q¦«?ž(ñˆ~³?ŸH{+àҕ?ïôM‰ Æ?RØ[="˜? îø3?"߄þ•?UGÀ¸Æs?R)¹nr»?ïßq¨lxØ?l´Ô!³?WœÆ¿S|Ô?S笉ÝL?d¿ôSyѵ?eÏŽQ5Ø?ï:"÷(ɀ?ˆg¶Eí?vÛ££·kn?gaÓ€Zt?'øx-U|?‡hµ©£/£?ïÑb´¼Eý?s²€SÎ?Jé$¸n`y?PÂÜ̲ÀC?sñ)c»6?r%f{eûAGN3FGL J1809.7+2909@Kás 
Ìã@5F(ÿӊVÀ9
3èdØÈÀ;Lü~¹D?剞C™Õ @×Ú Ÿó?þ}a?5¿Ûéß¿Ø
‡ñ"޿ۊIþYj]¿ÜÜÇÊ7$AGNbll?ïú,A¸˜?<{˜8?9a×ç;ÙG?2(‰Âí"{?5¼ÄCÌÀ†?-B¶õ±
—?ïgƒ/R†"?ž0œÊ,?|þ—Ååð?x}ã…HóE?‡Ð4éÊ<,?šrâoÝo?ï^‰Û?€ætR^?ت}£ä?v?ŽXaü?‡H°"'þˆ?uåä…à†?í"n‡>z?šÝ8ÁÕ?‡ØoÜöh?\'þ,?°a}Ê£UD?™ Æ™÷'?ïüC§Æa?0¤þ;¬–Þ?1co4«"á?'SAŽÿQ?)*óla×? o:èFR?ïÅ1•yNv?Î¥­·¨_?h®fg¸õ?fˆâèÇ?qýž]?|¸‰FÙ¹à?ï²3øf>ß?kͦ"?rdùô·N?`Yí0?t	ëgGÝ?_DÕ,LÑ?ï??ö»Ó?|4}.U³#?F¦HyÏx?dÑ¢ëÄ?FW˜¼P³?xÆù˜l¦ÒAGN3FGL J1809.8-2332@^_±ÁYÀ˜Ÿô|"À5†·¯.VUÀ9Ñ쌅´à@E»ÕX·|@MØÈÙx,@®'oXÓV¿Õ.™1%"5¿à¤Øðz/¿å6KÕQ¼Ç¿ìÆ'ŽmÊPSRPSR?K§ÂíÐC?ÒMT©šl?ï±6» L?‹Êsϖ
?ƒƒ¹ÆPU?‹¿R÷ÚÓ²?˜ŠpžÞ?W%‹@a?ìg½;Ü
?¸8MߒêV?¼º0ú#·?¸Å?tV)¬EŸ?n­¹ œ|~?ìÃME"E?¦_—Ö{X?¸œÀp—•?¦Ì\kd?
Efºnڀ?ò$žLý?ï*d~@?'¦ciwa?š¦Môÿt?'Ԟ?€$>ó,÷€Ük?Š#s±Åõ?ï«"àw?y¹×y?…-¿Y[`Û?x4K	‰Y?À=CÀß?EòŒkå?놥ìÁ½X?´D±åÚ?Áâ°Cª#Õ?´GEócÁ?y0å£Léš?€=יáëP?ìÌæÙÏzã?¦Þ®†®8?¸º×ÿFL?¦(SI<Ú³?.ÈZøHm?îC"cí?ïêÖþv?Ž
­Ú£Œþ?Ÿ3¥¸¥':?Ž‰¥ZcPSR3FGL J1810.1-1910@&">'âÆ?§Q*?ô«œÀ8w~@w¿TÀ9ÄõǗ٦¿ý~™Îr¿:@œˆjÈê@ÅT`)‹j?ïKæ'øm¿êý
!P² ¿à9õÅšç¿äˆc`øh\OTHERspp?u¾éø;As?zî4#ZP?NFå°\?Tの6?ïÍ\L²?}üxÞÑm¯?ж:^˒e?ÒhÒ})»?¥éÍöƒÚŠ?¤{h è½J?æFEñ?·•?Ñíkö¼?ÃÆ0•7ùÛ?¬Ø+Wu†?­³½†X«/?›mK.'ë?é38>¸f?°S<*¨ ?ÖTªuΨ?͆ÈqyŽ?:àéŒjZ?B;ƒWûSÐ?äÒN¨í´?͉eœ%?l'Ü¥õ'ù?pçâãF¯:?W½ÀÿßÕ°?pcÐéÍÈ¥?ïמBÜڝ?{ׯ°–,?Ý"†Tdӌ?Õæ")_lD?©,`K¾F,?¢‰‹%)ފ?ß·í¢Z]o?Ô})•"k ?ÊÐò©N?®³õ†"s?°ˆŽr]»S?æ'NTTt?çgyõ!b?°â‡ðð?Ø"±'LA™?ʋ•´²¥?*çypZË?+í«#°Ýœ?ãìøü"W?ʌ#þüŽ OTHER3FGL J1810.5+1743@FNÌ W"ý@0Îs`Iì³À8…Í!†b…À;Q€J=:ô?ýû%Þ
¥@––'7þ@ÅN¢zhÒ¿à–X¿äjlÊ9¿æÒS¬âˆ¿îùU=8ŸPSRPSR?£3pGu;j?£™á§ #"?h¹°n?§·¶¾',!?
äÁ%pÈ?‰&Ù*°—?—›ÉWsð˜?°,qÏ°iÛ?ìsw üWˆ?¿ý?Ü8ût?¶}T£.?»­ø5Ü/ì?È_…kå+h?°½îÀ­þ­?ç³<ã‹*@?³ÂÜPQ?±§
&1­?™ˆsí½§#?ªÇ¾ûÉ?—éœp¡n?ì7gM¹i?§D	-K?°ãó¸|'T?¡¸ù}§B?©5Eƒ®%?²3€HÛS2?î-½óñ‡?³î	ÒIŠú?wKۇ?…¤G=Cfä?§U¹ÔyHÔ?´&Ê®0ø?ë"/¹ùWè?ÂmTם¶4?·³¥FԃX?¼eh؏+_?Ó^s1"¼T?²¬å‡ÿt?ä‹t8Ùe?³Ë"ż?¬U%ü\ë?˜s»÷X	Ù?ÀììZK@?¢—7´?êP¬»è×x?¥èЂq±_?§A'ÖYtƒ?–º²Ñ ‡zPSR3FGL J1810.8+1609@E"©Ÿ¡—@0$™ù;À9Xˊ­mŒÀ;Zˆú%7?ãp+¶s@#»DLÊ@ۇß\òI?ëLøWÙÊ{¿æ/™"9ƒ.¿Ü–æ°N¿æi$nÔ AGNbll?ïæ‹Ôx×q?cŸHèâ©?XnÍ
²Ó?Rª18$"A?ZæçôO+?Zàið=?튟Úëm?»c(eÇ&'?š[uJ¢Å?Ÿ]†^w†?ª(G¨ÓK×?¶B¤{%ñ?î¬N~#'¢?"šÆî¦N?Ë沙H?' ñ2ó ?š¤H6_?vǎWC?èÈÒé鵈?³*`·söÒ?¨MYQËT?œ"§rœ?ÆÉ]ñ;°Ê?²Ñô¯ù?ïø¨vx¥?IR8Â_?@'k×jú?8, Š
ûy?;—€¤>u?>ç¶D,È^?ï.	i¾¾?¢œáUM˜?…§µXjcò?‰!uï7´?ŽÒHT$}?›1ÒmÈ?ïtï¼Í?}éqîŽÏJ?€þƃ­U?srJ8ÿe?ƒ'k‹?tÉÂr8©?텎[J?—a#W?y?œ8"ߒ?ÛPBƒ,?©‹Ýú:§?–‰í=Ö[AGN3FGL J1811.2+0340@?¢æ_E	õ@%8žç·4À9Hê7.jÀ;"nÞ,µ?òî«¢°š@b}¤ñfŠ?û\zßð&?ïâ]¨QÃA?ÃT…µ®oŒ¿Ð}‡0Fªð¿àå…é—†AGNbll?î'oó˜?¦Ç¶d4ð¾?¤}aÍÌèV?Ÿuk1¿O=?• N†Ï&>?–1ÊML¬/?钟ÖÝê?ÉÔÒïjuY?µ?1LHðï?»·?¿*Q?¾+Õín??½Pê?éÔe½Ÿm?®vF|gäÔ?·íÛã¨=?¢f³ÆÊý?¹nö2ÝÚ?¦³×sÉð1?ä«ÛE`‡T?½ÜS[$r?Ãd³Ëkp3?µÙ
±Þ"Ï?Éëßr|?¸ãßU>	¡?ï(ÎôÖgf?•ÛÚÂêÜé?"×^?Û}¥ÙT+?{u(
¡¼p?|fKòw?ìЉä߁õ?¿¯â*pÜ?§,[¤Q¿¡?²zîV_?«Ë'?²Ý<Zƒ—?í%üÇøbä?¡F~¤î?ªA‡H"	W?—\ŒSþl?£^¬:‰}h?"§ˆþÓ?ésáŸÓ֓?«C®"Ñû$?À´1±?¢Œª£Ñ,¸?´'Š #î¿?£6PŒôë[AGN3FGL J1811.3-1927c@&Cù¡A-È¿Ôñ·€
IÀ8iǾp¸À9¼ÑÇÞPƒ?ìÓNà҂@לã{@áŠÿ¢âî¿çOhË?ç~œóÁ-\¿áú©êIµV¿èpË¡ÖªOTHERspp ?—Ÿ»ä†ü?™ÛÖýh¦&?Ç%ç:ŒBï?Ç£i¯¤¦?éyˆYLÄÌ?Èf6Lº,?Á¶1]y?Ë4t7¯•?҉äLg¯?Èi½ø_?âwEì?Ñ?Џ7® šr?Ƹnyé?­\Ö¡‹ G?Å°X^!.µ?¯©Ï³N ?åûÌOày?´ ݋¯ù?ÁçihèÜ?¾úN-h ®?×güíÀ§?ÇÖzFS\°?ߤN_DÅ=?Îâsu?'$æ*?Ÿ¬ñrd?ÊiÈ_n"?Êe%¯Î ?èæ]4Â*?ÊÑr¼"×?Å·ØÁD$ê?ͽ¥34?Ño½"Âç"?ÁEþ<"¿?áÚ+M'ü?Ìei—¯oÖ?Ê¢6"DMÀ?¯/ŸØr?ÆÑÚ]PŠ?¯Šdкb?ã£*dW˜m?´7á
¹Œ?ÃyÈêŒ?Á}Eه?Í âœ(%?¾Â&ãf
È?ãÑÜ¿f»T?Ée¥$«õ¬OTHER3FGL J1813.4-1246@1>`ºTû@ˆ•_ùõÀ6¹"ñkéÀ9àЉð@±CÄÐÔï@ÜúE€èž@68õ¿à*¿Þû‡Ë:ü¿å"P3Áoï¿è @*8n¿îE;­nýSPSRPSR?h=•|ök?rŸk2°ƒÏ?è S>aR?ϾÍ¿"?ͼ² j?ϓÈ-o"¥?-2/¤IK?WN€'ôä?ì±òͬ4–?³ <;"«£?ºaÐ{>Jû?³"(_*îý?¢([Æ}¼ê?–´:M¼s?ãWfzù=?ÀP^³È"?×(bÙ	?¿Èü6ò°?(æéý~U?-AѺŽ•™?î8ólû?¢§=Œ¡=?¬eÉæ¦?¢ŸŒY·xÊ?>Û¦èRå?LÕM:9ü?ê¨Ò˜Nüù?Êvf9ó
?ÅMGË4‹?Ênf§¡;œ?R¥Ø Ï?m
/Oï?ì~·2±®
?«êFbîj_?»Â6,%'?«Ñ5¦á?ª#4I»?ŸP£¯®C?ä'goa
?¸,w@ùüM?ӘÎґ?·|f—‰€?3=º×{â	?0bD.ŠW^?í·…½Äœ'?¡_yÉUÛ?²0"U¡—÷?¡V¶ay¸@PSR3FGL J1813.6+0614@A»®²@&x¾áQ¿À9JEµì¶wÀ;:,XN?í¡Ô¬rÂÉ@st¤íŠ²?þW@-†?ï©
o6¿ÃWû'e¦V¿ÜPMR÷§J¿áî2|÷CæAGNbll?ïð¡X)â§?^uOþ"ÿ?JÔ—L?ONU³?QSB›#¾?S	³¬nH?ír¨3e]'?»mj.Ѐ"?–ù	ëSZ?¢/34è?­XûC؜å?µx΄ô B?í§æ§¥‡?žðiöC? 8Ÿ›fM?'sk°ÈÍH?¥I‰æ'Å?–tÓdâõ?ê×{Ã߂ ?®ÌñBŸx?¥]±ýaÂ?›N2a'ím?¾·sá%?«ØžÐÛ½:?ïú[Ôù'Z?JùO¢ã?8ØÀƒ©3Ù?AÀþt+×?4H—p
X?6t4)Pr?ï8¥^¯ôá?¢"ô¬]a?Tþê–3K?"*†ŠtíÑ?@Ô¸Qá6?˜zÕéV?îä°Œ,|?'NuTÔ?'²Óê\Üx?‰îÛ{¢t?'·)¤"?‰µr:~?îA)dy?"L9ɸ5à?—""y$mÃ?ƒXzÊ\i<?¢Á«.ã?'s†½ýY»AGN3FGL J1813.6+3143@MU§€)Ú@5Y‰?¯BxÀ95†S€À;…¿üñý?õÐq‡¿@ð`±¿Ÿ?ú­ròe㊿ÕWøÿi¿ß¯ˆ:Ãí¢¿ç(´Ù¿àÇæ|²iZAGNbll?ï$>^hÔ?–€}í*`2?'åŒrz×ô?'0žr5@m?ƒ%O{+…?ƒîÞTg•û?îG$=Y?¹"2P›?Lø]±T?¦†Z_}X?Ÿ
#«]¤?±HÉdR?ëXˆž¹Wê?°@£}*ö?¹}Ê+î×u?ªzCX¿?§{á¸AO?™Tgâòò?èIä*—8?¶LãxÇ?À#û-™|z?´[kýeW.?½hèTpMN?­Çҫͽ?ï½®cw–?€…Ô
"?yŒí7݆?|ëٟD†ž?^o"tÿ¾_?[±P
'¢ç?ï9Îj±¤¨?£˜E_eä?Ší ÝΰZ?"ÆÃ)}*b?†ŸDrX‰š?™½(ãûœ×?îq¾*¿ê?D$u"Òl?§-ƒÝ‰w?™"w»ë'?¶É9Ì'×?…3ð?ì÷˜¥¨Æˆ? üy·ÌÁ?°ÞÂÙÞø?š1ÐuØ:?'ß蒸ð?óH@ôWyAGN3FGL J1816.5+4512@R6¢Àh¡@8Àæ_E	õÀ9"¤úö«ÃÀ;µ(Ùº?úDن@p…qœ@äe½Ÿ¿×-ó´±è¿à0Pÿ³0¿ãꯋ?Ü¿ìÊ9­~[ƒPSRPSR?'tů	2þ?—þ´74?ï6þÚ;f?_'1§_-?~­|ýíA?~Cã[£)?ŸÇƋf¼R?ªWM{IR?ì ´ÊÜ©?ÂÎÝ Q5?·hŸ9ž?À!'‡'?³]á˜Çô?©44€‰T?é3ŸŒJÌ?¬Ç¶n?°üGØ&Š=?˜†Á(	ý?ºÆbzsŽ˜?¤6¶ëüø?ê¿ô̒Œ¬?ªÚµå÷ã?®sî>€|?Ÿ?T›çk?¬¼¶DÄ+ô?°hF4?íÑϖÅn?±ãczY?ˆËrù"Ü?†f'
R?·JƒXX?»¬-è=
?ê&»òp0¦?Ė,0'C?·UL÷?¹ý#µDx‰?×à+±+(?µMM??âã
Ý»?µ6ýÀ…?°P8Ôª3<?˜™'~@yw?ÒµäAÍC¯?«ïvæ3T?å–¸pkÅ?¬8Õ­¼Ò? ï'nÚ©.?DÈì+ePSR3FGL J1816.9-4944@u† fèÀ.X­~«À9ülhÞæ«À;Ë?'‡]?ö
´ynÖÍ@·Ýª»ú?í{xg«ñò?ïGãmðjÙ¿Û0!œõ¿ååÏA"•–¿ïþ'B)'˜AGNbcu?奮HZë<?ÌýɑPlK?Æ4ퟢ"Œ?Ľ.MŠS?Ã4Y<Ëý?ÄhWÖhb?à›œ'S]?ÒH½	Ô?Óä½ô»?υQ1º¦ô?ÇmÆaΧ?ÃyZßË?ÛãçÚÞø?·	Ûõ—mÜ?ÖqulØ_A?´ÄŽ-}«?ËUEp'Qe?³
(×Ù~?ä•M¨#=?ÃUüŸ+?Γ03y?Àé[Iù¹?¾/2XÓçÚ?µ†UÉO¶?çs4 7ª?Ð7Çà‡rX?Ńß	ݛÉ?ȨôÍ·?¹^ èK?ÂÛ!¾¡¿?æL³Ø'±Q?Ñ«Óa«/ˆ?ÊGçºR»?ÍòÃÓBN?¹Uhô'ˆ?µË[<Ð?ß÷-KÆ/­?·‹šQ)?ÕÅ¥À?´/À`MŠ²?ĆZH\ y?°ú¥ÈË?ëcÈFÓ?°Æbòü$?¾À_¸ï—Ÿ?«dˆó\˜,?¡É••?ŸŠ4x¥
AGN3FGL J1817.2-1739@*Ç$ß³Y^¿æ-£€Š#À8@5¾þ­ðÀ9î'Iü?óEêmFª^@ŸŸšm@+/ŸÕÈÊ?å´õ«gâ¿æ˜"üS£¿á8½`É¿èš´¡²ÂµOTHERspp?§i$«·ÒŠ?¨æëbãDË?жޗC/?ÉsE\€‰}?æ-þi윐?ÊT3Ž±3?¯¨övò?¸ZvŸË`?ÀÍv|g@?¶¤L"ˆå?éӧф†Q?Áö'ÙaÓ?Åî;ÝPÔ?«wdä¦Ë?ÇÙ)‹ƒp&?³Å¿
š½ô?äÈz
ž_b?µ±ºğ?Àäà¿ÈØL?¶Àk4iY¯?­qÐ2û? ïLDûR^?éöÀ²üÛÍ?ºU7-Øo1?³eÉøûâŒ?´;¬òo|B?Ô[O¥•â?Ìógò"Áú?ãeÁ)5?Î5ÝV ·Ê?Àyò/?Åb":Æ5À?Å׌<þ|â?¶Ôr¡ßÇ?æk l>%?ȲõP›ñ?ËjBÚ×7Æ?¯µàÄr؇?ÆIúÚ'?¯/ـr'Ñ?ã'ðÉû…?³Ü³ÿ?Ä÷}Á]=?·4y‡Rµ?¼fW¼™<Á?¤˜í…Ö£x?ç5U˜"™?º{\×2OTHER3FGL J1818.6+0903@B¯¸Ÿï0@&¿ãAƒXÀ8¾Š¯ñʳÀ;0žHUh¿íû¨V@wEöÚ<w@ð6îÍ©¿ã69Àk¡¿ãÆX¶È¿ç.«'5>s¿ã+h¸óswAGNfsrq?ïã
0ó›v?eÚGaxøÞ?S0á<?Qç[±IÐ?cZ^¢ –?aà"Ö#›?Ã,?¦èÖB¯b?{if¿0eÑ?|a
ä¹îC?¡©a-"'?¥ËT1¼?îFø±pê"?—ŠS	û?"@ßz@¼G?‡)ñµM_?¡ð.d­¯?'ƒ@kôÓy?î€À#_ð?–I7X;=^?ZôE•>Ð?]ôÀŒ%?§&qÐD)?–'bè¤ç?ï÷´þ«¯?ROt·(÷ù?;N<‡×ù?8f¡öÒ0?C…¢ú~?LJ^Œ°qû?ïªiRvg?"-3Ó`̉?b÷ŸØ¦¶j?^ñ½öèÐ?€¿ý±0´?Æ"
Q?ïlbUJ	?€1®þw–?€€xsP@?w¯J'õ÷?"gÙY?r³î-ì^¥?ïžyþQ]?uõðø´?5¾*b…¿?/Rw1ÛJÔ?‡Ó[–°"b?uοrqŽšAGN3FGL J1818.7-1528@.ù"!bPW?ƒþèÀ(½¤À7söLø×À9 Š(Ž"@þê<F'@Ipû@?ýr9΂Úe¿ÃQ²º§Ü(¿æ>ÕÈôÐø¿è¼*2	h¿êÖ#ú±OTHERspp@?ãšþûF}?§ìGKÏÿ`?¢îÆ£'4Þ?±7}©?íáö½ê^?·—f–¨q¥?²é*E`ÍÄ?Àq•®?ÆJаm?»øí…1¶9?èUöV³ì?ÃÈ+#*®?Á¨%‹ÞM±?­£g7l‰Þ?Ïþ™oñÕ?´'út9‰?ã–P[âÿ¿?¸èVôk?®ÃXeý±?©Ðx(à½Ó?ÄäŸDdš?¹ç+Z†?èÚÄR'N?¾hWQ÷?§'¶Ø»?³¦KW9Î?©4Þ»Ú¸?µ»ô"×9?ìûˆè؂I?¿M½ž¨ï?É*ÉBm}?ÏFÄöGM?Ï)÷Œ'Ê?ÁŽdmn?áë9ÌCî?Ê_Ð	Ã"T?ÂÃpŠ&?«p"ƒÞz?ÒĜ҉$?±š²'Ð}§?âBA¶Xä?´Kð‰Š?­~UJ©)V?¨†Z
ƒ(Î?Ñ'äödJØ?·[‹$¸{o?å"(/ìN??»*f¥mIOTHER3FGL J1819.1+2134@H'ŸÀ$GÞ@0}>ö?À9å(¡ù¤À;Š¦8
‡¿¼KŠÔ&¿@'ÈVñSj@¨_Û÷¿á֟ÞÏ{¿ãè½YDóX¿äv'6+"µ¿²^B¸XÃÞAGNbcu?ï'ìI?¦ƒ%~ˆ©Ú?~Šä™þ?¦zJ]—ù?xj"ý7u¦?s˜^¿Öª©?ïu39ØÎ?"äé4r´?t ýjLy?'iZ5Mc9?ˆ¢²ÄyF\?¸Eâ
?îY±.-1^?"ÿ¯ªîM?•UEš?"ïÔ·Pè?Ÿµ…7«Ë?Šé
qÃìÈ?îôZüÖU?#ÝS¹®?W&¯e_Š'?`²Y¨¾×? (è	FÙ?Àؼ'?îN؀4C?Ì6%Ž1±?®|XY Ô?ÌA«,OO…?Y×C"`U?[¾CçGù?ï×É[NŸ?qZ¦jf"ñ?[Ïüø­G?T¹&Ð?ó1?jNÿ·Âc?lá©?4a?ï_½Gý"^?€V# Œ)©?ƒ}©îQ6?yú%eHK?""jgc?ll+£ýÄ?ïÍ_±&º?lã»'ëÙ?A®Bê@?<¨ñÍS_t?wWî?ïrT?kÔbÊÒÛAGN3FGL J1819.1+4259@Q©'ŸÐ€@7¸ß_vˆÀ:<³Þ¿=˜À;ΌQ²z;¿Öô&žáhK@¥²YY·@߃]ÿålòÊÀᐿî'ÜDÓ³`?ÚuYÂØÆð¿éü½ðˆ`.AGNbcu?ïë¿`þrŒ?zar=ï?8	ÈÏUAW?L4Æm®RB?a?eè/ˆh?wr^²Öß?ïuKM¨¡Â?"ïBÏzª€?}7Áxµè=?'7²t3?"KÊ^S?Œáÿ<uL?î;ȶÊX?•Ä/´¨¹?'(J†gáÜ?"F
½ú*?£¯OY÷›—?'€%ž,øÈ?ï4"ú¬?!á÷ãC4?Róýþb‹?dñe¾¹ÏE?˜M͔þY?œw2a]/^?ïÓò­øÝ?¬¿ÚçÒ<?P_SUE4p?ŒX¯ú£?rQÏê²;?¦žñŠUà°?ïÎ7µ<Ò?uõ­GDÞ?hX÷͵_³?gšT×2Ô?ioSwY?jdØPÊW?î÷xq'à?éÆ£Uµ?€TK·†
?r(pd?˜æ×Òôµó?Á!œ'«z?ïØsH™nH?r™þJž‹Ó?N?KÍI>?\âú'ý3Ã?oüä6\È­?l†Â"ýÞÆAGN3FGL J1820.3+3625@Oõð ¬ @5'â_ܪÀ:m&!Ò¸ŸÀ;ÓùrGE¿ã>ªCF7@x¹ÖÐܧ?ümá?¥¿æcÝ	ñ_¿æ¶[[	f¿Ö'÷6‹_ù?¾d´AˆAGNbcu?ï÷ˆãœz¨?EÝ\yå?‹yòꀭ?ý=^Îç?Mëú$®"?Dn™ø¿ÖF?ï­z0À¼?ƒñå WGÀ?n'xSž™¦?mÛÞ/<)?z/+t'l?¡-+n-.?ïq-HU?"TÇÌj£Î?'ÂT7â‡Ü?oW˜¹9

?•°?bw?€£'	ëÐ?ï§
kVí?9LƒºÛ?#Åo.Ôº?2¥T®¼w?…í\vDø?)Kj™÷?ïü>"ÓJÚ?/"¬·v?íBRÁló?ѝ¡©")?7Ð@Qž±?+±®V{|Í?ïâëÅéâ:?hû*Lí?Xa³fàZ?V¯(9>–è?`ã`e&9?aØxå?ï‡>"Øû?p豦Ëò?v­8ê׸?bÖäGy¦‰?'ÙÛNRòä?dݘ½^Ä?ïò†g/0'?P´ÄF"1r?

Î]W4â?Ì ÷­Ú?Z
ÃI³‡?P…Î}}a†AGN3FGL J1822.1-7051@t:gÿyÈÀ7.L`*ãÀ9õågÎEÀ;«¸ÕŸf?ÆG^™‹@EôZƒG@Ÿ¦ e¦"¿çµ¾t´ È¿éJÐeUË¿æ	c3´–¿ïÿƒ£žÃAGNbcu?íDˆù–ã?¾9ÐHú<?zƒÜó}?!®0>‰?¶=«wš3?½Õ+.ñžØ?ÞOåé\?Í)~|e^Ý?Óö½!?Èö%Ð…?Ët`$-ó?Áô®ªÅ2q?êó¿³gT?¬ÇË´ˆƒ?³Ë$z¢wS?œQWÐ:Y?»í=‰è?¥Ër±W¹@?ܐѝ۷e?»è[YÔ?Ò¤ˆµñ"?¾Ü§q"¸È?ÐÊ¥¬2´™?·äÕÓTÒõ?îR‹o¬­•?´±njR?nêBH5ä?s{§‹Š»B?¨è¤àÙñ?´pHûoÃ?é̝*Pi-?ÁÁv]ævR?¼K;'¨9?·òØO¤è^?µ†Ëq'd?²c'…*B?ì¥+¯8ñ?¡˜áA[¼€?ªìqÃ;Ôl?":o¤,?ªÂk'¬ƒ†?š-Š–‹6?èÕ寖?©¶ÀÆA3?½"JÊÿm3?£‹õ(Kþ¥?»½‰<C?¢,ø>g/>AGN3FGL J1823.4+6857@XÌm_êKc@;­5@S­&À9`žc,öÀ;Æ\>'ãÀ^ÙH0Em@¬àÑ;œc@DI€§…@¿ä™Wž'>ñ¿åFfËÞ\º¿ÞZ'qf¨3¿ë!Hï ùAGNbll?îîá/I3?"Œ(¯Ü?"@(¸îº?ŽŠÎ•C?þi›
Þ?†w9þë?ï†Ád±&ö?œ}
ǾÅù?wéq¶57™?†æWäýÍ?'Zíñdx§?•Vš†øƒê?언ýsD?¤îxbû?­~èùŠ7T?œoh.Ý ?©‡3œ?•QÿsŠˆ§?ïh‹š°ùe?'Ö@覾?Iµõ£†~Á?aX´°ò?' Üû`a~?'o™RèSh?ïªjqZW²?~A8Ÿ¥Âˆ?z'T_`?v^"	ì<?p£rÛq¯¶?jՇ…Á²ª?ïÜ´è:͘?tö	X¯ž³?_
©~Ɔñ?hþ­Ô¤\?cÄBö°Ý?g¥0H?î±^öõ./?"©WÖo?™0Wjɀ?Ž˜àìQgö?£ÊÚ£?i¾Å® ?ïäDõJx?p/Ïfˆ1×>ôp0>¾)X?Gº21æ?k"Œ&V?p,•¢M¤!AGN3FGL J1823.6-3453@vjá€M˜9À#Þ\ÀjTÀ8ƒè!¼é*À:ۚânõ?ì÷lN˜ûu@àóÇ™?ûùI þ?•jy³íz¿Óoò:îé¿Ó¾Òƒp'¿Ý«xÊþ&ÈAGNbcu?í,k"¸¼ ?¯›ÒB¨R6?"Qe.u6Í?€kœÇ{ž?±ÈMžœÍQ?ª‰ÙBˆ?éiïÝÈóy?ɼŸžýlä?¨@øí·ßó?­33QCÈ	?ÄHM7@^?Å(á;ªâ(?êÆ9iûh¹?«pϨ¢µ?¦!°ëK?"'ìڑäø?¾½\=(æ?§¢äãâ?䚓âu€‹?±Ž"Åpí;?££§ù#"ú?›¸Mai?ÔVc;0$,?±Ç®jaÐ?îše›ÝŽ? ÙM+z3?"÷\yoÛð?€2À3ƲÖ?¡Ï"ZŽ?œiÿ£Ž»?ìÀÅ}"?›?¼û&Ñë?4´Ù	GÝ?§¹"ÆxÊÂ?²¬¦âc/?»ç㜥›8?íèUN—E?šô"¨—&?™#TD°,?‰Vp²Âû?¤éþæL?•(ePœ
?éꚴæjò?¡é)÷5±1?¦?áŸp?ŒÀáwUï?ÂÅÐó粛? )òõXñ¯AGN3FGL J1823.7-3019@'œÿT´bÀŸ!€nÅÀ8ÜMÂ*²[À;&œKû?ì)¯‹žY@
þ{uí@yoÿl\J¿Ò>ÕÁp«Â¿áôôç0¿ä8úC8Ë	¿ê'ÖwŠ?PSRPSR?àu¹Î?ÇàY…NÖ?Î9ðì;Ó?Â[nIÎný?ÏÊP;Üõ?‹m‹7šæ?×4¬3hüÝ?ÎF¦§
u?фå·Ig?¬â/ï?×Fn~¹¼?Ç46ƒSm?唎="¨Õ?³žHöîþ3?ƛ"_Q`?®oÑ}™Zp?ä¬aL?¦gBôæ)<?ÑY}^>hŠ?«{›AdyQ?ÔÌ3ý*-?²àtUòÂ?ÙÚN¤—"I?±§GÏì€?è11Ø·‰?À¾_²Ô9d?½³ŽýÎ?´eDŠ@Å?Àa±Wȶ4?µ+•Ÿá^?ã÷Ù¥ù#m?ÐN·âɨ?Æ¿y'3K?¼Ï¤á~é?ÊÙîô??Ãåì•j
?ëÜ9"vÅ?§@ó‹ä‹l?³â,"åS!? 'sä'd?ªx¿Âjw?•wße=¸?àZa>'ê?©™=CÑh?Β4*m×?¤¦èó°!­?ÐÑ£m¥A?¦icmymMIXED3FGL J1824.0+1017@CŒß€-·É@%g‹_D36À9®TDZ±À;a~B%>~?óîÔâø@²¦Ú?ÿ×>€C\K¿·O£°•Ä¿Û»vžAôí¿×agnN<N¿îQo3òÿDPSRpsr?Ì¥B(][?ÁR/±¸8/?è*AR—?Â1xÂxNà?•Î‹óü'?"ûç?Չ`‹éX?ÊpÛHÕK?Ú#.ൄS?Æ®TQ;?ÐSq
«±—?ŗ"ë
?Ô"gk?´¥ª\?âVOu'°?µ»Í‹  ƒ?½
Rüá_?¢Ü0Zb?à5<Y;td?¼I:ÆûQš?ÒÕ1)£L?ÁILî"æh?ɀ¬Fß&Z?±êM˖À?Ձ²WU§Q?ň+4®€?ä¬íŠ÷.9?žfꤊ?'G)*õÊ?ŽMÀe%î?ß|º÷É`î?Ê¢ãÖ¿?Õ=Údµ1?Ä{´MÏí?ƊÕFE?¾ÚAÄ4f©?àõ\ë_×M?²t$c8hå?Ù>åèk}–?±Š#6QOó?³Yå[¼?›/»è¤æ?äe;š¤ M?®…†w‰ì?ҋ+U?¯|n!²—?²©²zç±?–Ú®ÀOï_MIXED3FGL J1824.2+5649@UnGßþù@:ÀÁ%ÐÀ8Iò×sÀ;‰ùÖñý?趃Q¹±@%͙ü@@®?Æ ¿ääÛ3a=¿åŸÿ«±¿çQIß/¶¿é‡pu«ÒAGNbll?ïúø¾˜?<äßÔæÁ?@›»qÅ?8eñŸ¤ç?-?!flê´?!Ãw­Ѭ?ï¥øŽ,å"?"^Q¢ê)?roÊÙN°¨?p‹'!¬ù?z"î+²i?€¬·[³ôQ?ïMŸt‹(?€¼ö[Š–ý?ƒg1ÆVP?v`ïäå?‰RfO kß?uœ	~`†?﨓Ê5¨?"7ØBN"›?ca–aîu?c߆ÑÖx?§ÒÒØM?ƒA¹KàH?ïüo—Îz?0؏q0Û+?5:±c?Ê?-:¹é:án?#(LLÙ?Ó) É?ïÚåbK‹?q;–Mn¦±?_cäÇcƒ?V6r¤€‡?ei	ˆSè?lí
"ë?¡}ü?råC`3f?wsQ™àÇ?k€°¾Ó«?z7«6ÕÍ"?e;:Q³?ïï"ó$¶?c=tø ö:?D‹úWì;¥??r'n!a?V±ò·K?a}úÎùäAGN3FGL J1824.4+4310@QÇß 'á@6ÙÙb¶®À:Íú8?ânÀ;øIlÊ.?ӕˆª€i@
"mã]\ý?û˜ÔÀ6;{¿ïÐwwclj?ïëé‹Û|#¿Ü P¤Õ"N¿×Œ0Nk6ÊAGNbcu?ïí#Pßbô?Y¥£ŒèSb?C5©	¡å°??cC$êùØ?\Š8as?V°sOØÛN?îv\_S?«o¼\"hÅ?™V"WNV¶?˜üÿ'œÐ?—ÝïÆG?¤ˆõ[²x?îÛçîU"?‰‹
Ëé?ûçë¬Îå?ƒ0ónËZt?" Çîh?{ŽÙéí!]?ëÞk½A?²FÁ#"1?¹m²æë³¢?±¥·ÖyÍ?ž{¼½IÇÖ?œH½U'à½?ï÷Øòí??HT¯ÊÕq!?0ác
¨æ?*c	Ì`E?IOë"öžc?D«WŽHE?ý£¦°?¹šQ5¸Û?w#ç¢Nf›?w_3/Ä÷?||™‡¾¹X?‰|	»ÀŠõ?ïgC‡$ˆ1?"cNqc®?'¸YF?|!nÄ?"#eÏ)€Ò?iÞP»ØÖj?ïýƃ¡O?‰
3Ô{"a?–<Û81Õ?†‰¥?y
°VoYq?pœ62ƒAGN3FGL J1824.5-1351e@1'A@<02¿Ý`às%oÀ6Œn~bÜnÀ9*Š§ŽNã?öWvšÙ@'
äµvÅ?ËÝJ9pJQ¿ØèPKqîZ?é«\ÚÌiÐ?à(‰¡~ëC¿Â²_8IÈOTHERPWN?"ƒxqï?«®° #ÿí?ÌÛ¯¶¬?ÐVþú1?è$û™á4…?аD ßÝ?È~aîEK?ÒwéǕ'ˆ?ÂqÑøõc‰?¿R÷ç¶:Ã?åCóÈF*?ҍYwô?ÆìAÊìV?°'¾)Ù³´?ÂìXÀþ&?«i"êÄjº?å‰Ùš]a?´B_®Ë·?¿›{"k¤‹?Å"D®ß–?£NöÉz¦È?¶ˆ"¼ÿ³?êס!MW¢?ÊÂ0wÓ1?p>¬e/£ì?ˆüs|¦#(?ÊhôÙA‹?ÐEÑM_?éE[*oÝ?ÐHÀäWÍ?ÒÑè¾M‹­?ÔeeˆMŸy?ÈÑA1šú?Á†#Ιß?àbÅЌÓk?Ñ¢*¸Ìuö?Ñi«5´~?±d—"|l?Ämà¶Â'
?©Ù_VhN?â/²7u7:?³}'‰a8?°Òú]1?¾Ž"V3"U?±@Žªÿ·?´ŠqÂ~Ùê?뽕Å#¶?ÅíRëס_OTHER3FGL J1824.6-2451@DHÿÎ+òÀa'ßÂó°À8E3å	ÚtÀ:Û5ƒo‹©?ü×È j® @ ½Ã@@"4"¿Ù­`Ç|<"¿ãs§ªyª¿åýÎl+™®¿îb!%û£`PSRPSR?rq۝`?p¸'š‡VQ?êCeæþk?Ãxù¯¤W?Æ`7õËÛ?Ã;5˓ç©?ZÑ#0XN?i"³£nü*?è×C¾ú.ã?À<·&®{º?ÌmNÚP"?À.ƒOoÕ?µù=½«? ¹:A'È?溗øH•_?²üD;¼A?Ê߬Þp?°ós3¤([?›mA|2?‡o7_+£a?é÷6´-TÞ?¨Œ aÜ÷?ÄÁW…šU¤?¥¾¼+Ôj?'øJyَ?"$XQL/?蹤½þ'?Ä?÷YñÁ?Ëéè`_?Ãú4.ZÜE?v' ›Fé?…|—@©'?é–/¹"?¹"Ÿ¥íÒæ?ÉM–>xê*?¸r
õ¬ˆí?Ð*Ð]Ðë•?±<w6QÓ?▗ŸÕ"?´b""?ÅPÅŽ?§U¨>'?¬kžWÆ?'¹!Èrb-?êç,ŽB<?£h$®?Àðˆdy7‹?›}ÍòLõ7PSR3FGL J1825.2-5230@udS_ôöÀ1w?› 'À8Óû|ÀÙÀ;Z*¤ï82?õŸ©X~qJ@óE$Í>ã?þTK'ôà¿Ñô]%†2›¿ä]rÍä
<¿æ˜ëK#¿ä±Çã%AGNbcu?ïﲈ†i?UàõÌ<Œ?@
)½Ì??A¬ë[Â?X•à›n'€?Qc¯añ2?ïj) H›‹?'æžps#œ?qŽÊðÀþ&?~¨ð—2?Œ®2nAp?‹±×2iOH?ímŽ"_? ŒK¨
{?¤–àl;èd?"õ0WÜkî?¤7R'U?–=ÝPëb?ïx"ýé?‹œ	{øˎ?Xyæ9(ü?^·ÏZ]Óø?ŽËÃòºpt?‹^Žìò{?ïù©0)WV?C±ù1ÞÛJ?3Nÿs [?0´ÜB0vŽ??g8?ò"?;;©3ŽêÜ?ïɾ8
?y1o‡
1?\É h,ô‡?]ˆ²Õv‡Ð?sî‰jiÜ?t%|Š£=?î©Ú5"àê?"úÃd ø?™'öpV¿?Ži›ÐìÇ?'1Ã0;¾?…Vq­•šŸ?ïá¡ïd¸x?gÙHá9N'?Pœ=wû?L:!Z¥M?fP0µ¢2?eCä©åAGN3FGL J1826.1-1256@2Žwß4®]¿ØJä@m»À5š'3K†çÀ9y[ñ˜^@	o_F6›@™åX3ô@ÃTUýŽ¿ÕmW=mc¿âš !¯¨¿æ嵕3êy¿îj+.¤O¢PSRPSR?[øþt"N?óRáæò¸?îO©ÑÓ¥b?¶V¢KÅ?ªù4æâ#?¶áØc'?1»¨y¯Z?^&œár'F?ìr-<Ä?±r³žŒúM?¼\ÛÖ}%?±x`¤Z'É?vñý\ŧ?v†þ"y³?ꚑ:ÇÉz?³5-§`µ*?ÄÞ26RÉ?³$4̪+ý?1=¡ÿ~?6¤OhFù?ì¹­¢ B?­CUí¬È?º!"Ž^kà?­3/º$K?[>½¼,ù?	-9'fÀ?î®N?·×Ê+Âj?¯ǾêÙ?·Öt™Ä‡?8¤1瓤?XµðÅØðO?ë–M²˜÷'?±yJ}iÕ?Áš‰ckŠ=?±k^Ž/ø?xߏ××Íq?€OmD‰Ä?ê‰ûÂê±ö?°óϽþ?Åvë[?°¸ñõÞ³?0y÷dóó?,vI¶jÀ?ìïÇzÊÄ?¦^ŠOÔÈ}?¹ÒÎoS?¦_By¯ë×PSR3FGL J1826.2-1450@0â³ÀŒLª¿ô³b ‰!ýÀ5þl3/uÀ9ÂQvYS?úȉ+bYf@º¯¾Ê@å¿ÉY$ß¿ãº/§î¿æâƒb ‰"¿éÑQa£Ê¿éh'žùTëOTHERHMB?dB >?}?
™Gúj?Ö_?'ßbž?ÑQ[\ï?äŠÏ-òxû?ÑPŒ‹zXG?aî+zUÔA?v"vž‡´ÿ?ã7Ôaãí?Æ2¾]9?ÙlzäÅ€?ÆQ´ÜÖ?ÄGƒ'à?©=ŒÛ²?Õ¾È!í:«?·£¸|U?້Z²?¸ï5Iå‡?ÚÕז?‰)"¥ê?ÛÝr¦N´?œI;!-?áŠpC+p>?Â`fã"?…Ï"@àÐ?ˆ3ÆM{?Û¼¿wé_n?Òt	"y¹?áÊa÷ۈ?ÒÇGýš ?^Ï׫‡?q™i}c?äF)ŠñhÁ?¿ê(ÛÉó\?×Tݦ\?À†Ñ|?Åñ,þœl?«¾by7rŠ?Ö¦†µ«?´i±ð3¡?ßÃóùü?µßc~‡)?›OªíÝ?"[ÄRÔ?ÕÕÒ}nsY?¹æ?ås6Ù?ä:™p¡J4?»Q·Ã%Y+MIXED3FGL J1828.4-1121@47	 :2+¿ÁËTŸþÀ7×ñ
õ´À9×!éBN?ö*mþ¶)@P
º?<@kÛ±í¿Ç´5§+Óm¿çN'D~ˆ¿ì½­?h˛¿ïÿkOÚ2çOTHERspp
?´ÅvžHÑ?»Ã#««À?°œ{m«÷?¶¹|K˝‡?ëd=¯c‡?Ä*©²ý?]%t?¬I™åºq?Äú8XJ?¹µ»,`?ê˜IÒâ?¿‹¸IKè%?ÇNbtÐr°?°QaNR/?ȏÆÅTf?®HÒXÐ?äu±vÉÐ?µ(kg®Å8?¼©µ4n‹?´ƀh¬M?Åe(d^?ºX9'rÞÅ?ç$ ¥@Z¨?ÁfEñÉ'ô?Ã{w²5".?Ä}"âÐf­?ÁO(ø°Î?ƼìÔmï¶?æÍXônÁ?Îúø"=ù¥?­öpuc"?¹ÓUE4p(?Ëÿñ8"A…?¸²ÚfÌw?ç ¢:¹­?ÃÕäªÔ?Èk\ö·=*?¯["*Dî?Ì|@?Fx?®~™ "?âÆ#rB_?´3Tß3	u?ÀF×E?´±y]º	?Å%¡ÅbZ?¬zP<Ô'Ò?æ¤áË%q˜?¸~"¼ÔyOTHER3FGL J1828.9-2417@!Ž¡à×ÀÚ{þÀ92t]ŸîGÀ;r«G¿ñàÝ"Zrè@U<Kv?ÿÃÁá6fD¿ë9Ó>'5¿ÑÆ3îˆÎ¿áŸ‰¤X
¿Ø{Úp=CœAGNbcu?í¼ÝƒÑú?±E¨jg³á?tGÈ¥ý~f?oSY}yšL?°Ô—]F…Š?±êôޗX?íÔhIaë$?µ.e‡
-?†@¡Wix‰?'9³0í©?­)SïŸ?³CþʅP¶?ì6ÅJ2Ý?¦›¼ôÊ?¤'´Ž`­?""Ž8?´ý/YùŠ?¡4KþY'j?ìþ"î¬=?¦°VÒ"5Û?VN#F§"d?V¸ҏ&ø?·²'ý¯t¡?¦Š@>Â/%?ïWü6µ?Ÿ[Œâ‰Ê?eïp²|`?a‰žéÆH?™·͛GÒ?žàÅwúÕ¢?ïF1o¶á?«¿T÷Н?p#.wôn?qX(¾™?"9S¿·éÐ?š%A¸D?î¨ø&Sø?'iï»lÛ©?'-«Q†ÿ?¥Ð²&-?™³P"Lô	?ˆ|˜QÑ÷?îôÅÈ)W›?Švwëô5?9¬<¶/´+?1CDZ+2? €K8Çã?ŠJH >AGN3FGL J1829.4+5402@T·W?íUÙ@8Ê	?Câ®À9§0IAÀ;¶½ã$þ¿ÚFØRM;@´
Öó—<?þè`·Ð¼¿àjï7/í¿à—j,Õ²¿àº-°3ÜH¿ÍÁ:Áa›AGNbll?ïó´¿Ýž?H-Ía"?B‹nÏÊ?5f£—|[?N¡þ0¾‰Ô?B—Ó¸päÛ?ﭓàXV?…Ï`;Y;h?o¿`B'õ??mOÀtLÖ?yV_œ³?'ÔH%
Œ?ï2¼ë®9d?"Õ¸ ç2?"Cݺ¯¸›?v3Ëd
	ð?çfx|`?{ÀqÒÜ­?ïl-Ë?Y?"	O2?K†ÞëN`?L$"h?'ž¡½èI?ƒâT°ŽY?ïû¾í¢-?2
$Ø›ü?+G[FNáÔ? 7&4¿+^?4dêTñÿ?*‡§ÈÈñR?ïÞ.kù"k?lkŸZ"ô?ZÿlzÞ2È?R»—4ž?dQÞfû?g§+òWÖ?ï¥øê'É?hðV¦í—?s°I±<_?_ãâ)3·´?yS«Q똴?\$Fq®Œþ?ïå|3àµÀ?]eÁ"éÐ?1;Ý!WNÆ?$àR0¬è?h\P²¥Ò3?\¼ÇÖƒAGN3FGL J1829.6+4844@SNü_Ìï1@7|5_]]©À8®¥|%ëLÀ;™—û3èe?æH¢R(@eàÚv@뮟e5¿ãoÉ´i~Ÿ¿årcÎö6—¿æ 4=tU¿é¨e¾´AGNssrq?ïöjø=á.?Gpj^ã!7?Hzáf½¿ƒ?B}¿$kåÄ?;²{X_k?4Šš/ºæ?îí•ißÑ?¢^'_ŒÏÔ?±‹?ô?Šõð?j9Š?'H¡7%cÅ?žÈ.''?ïD‡ÎóC?ƒۚl;¶?"šw@ýké?xDÒþ¤:#?ŠC•KÄ3'?x4Uƒ¨^3?í­—ÔXÃw?¢&—.u0?Ÿ`pÝ?'­9ÎF¹?¥vrÿÐ%	?ž"§µŠ<º?ïû‡	ôöb?3"rÞE‹?9ò£Nj£?.Ö¤´:­0?%e~íc˜ë?[4²œá?ï›w—)?ˆHñ3Õ½?x‹@½Ú?qš]½ŒT?y¹3nh§­?ƒ/ãÐMû€?ïŸÂi¶@Þ?pÃôº¾3­?v¢ðâIU?`Ü×.? "?y{ÛÝ¿®?iû)(-Ë´?ïzÐpØ<?'œ¶¹ÍÝ?€ŽÍê5'?n°Ñ«`?€½ì>£È?~bŠh>!ãAGN3FGL J1829.7-1304@2ÚB×P´¿ó|ÔÂ^À8d"_õIÀ:&²ò0?óYœƒÙ¾Î@̼¥BÉ@öc«Kž¿ÓR|¤–LÞ¿Ù¤Ò}ö¿çw,ò§Qé¿æ‹(³OTHERspp?|ï¡hèó.?…Z€áQ?ÇÙÿBôO?ʱžöHØ?êj=Wñ¦?ËCHl-ó?²Ì<ɨã¶?»´Ÿ¾å?Ë b~­ã†?Á%çpg?æÞ_Ç:çˆ?Æv\ÞR[B?ÀWÅ©l?¥h"áÓÛd?Îÿ}¡ýI?³]'á9Xv?ä*/uRVS?´¨ 'jH?¾¡†U¢§h?³}§ w?Å|^"^Ä?´Å~Èq™+?æÌ·"4¢?¾XEž<8?x2ü ‡Ç?'e£ÈoŽ?Ä@íRu»?ÈþÏ
a$U?êÌA^fŠ?Él¹ìm?¾¬¹©Pé?Â[D
ø?Ìë0';xÉ?ÀÑÀP9?äGª?ÇÕp¨gEg?Ë"ù2†e?­IMÿKÖì?ÍHZYÆN?°Óå*Uƒ?áåz+ìÓ?³Ýjs69•?Ãmé6(ʾ?µƒ¿úÔ?Ê;~ú9 ?®pmþş/?䕥óçeL?»V=4¥	vOTHER3FGL J1829.8+1328@EQÅÑqw@%ŸàAׁÀ9øŽ½À;e×F£R€¿Ë×¹"Sš@
]|DÊ	y?ýîÞÀX¿è|ãN¦?Å"›-¿äž,÷b€0¿Ü£³Úž­¼AGNbll?îöN¥C_À?
J/ßY?yƒc>?3"?zkŠ"MgW?šÕRŽ_'0?™rê]u^Î?îš¹Cø?³ã]دK`?Œú§/í?š|êŒPZá?§·ªŸÒøô?¯ÌÝT3§Û?풢{âÆ×?–ž$‰Ee?™H HX‹?ˆØ	Ž¨?ª1ˆ7±?—M«"¶?í?5‰hÍ?¢€¸ãf
Y?'ºJªxX?ŠL|BaGš?±—Áe­˜?¡1š†ó\€?ïÉaÁÍ%ž?"å¥Á.Ò?Wj¾wºð®?`Ô¨Os<"?uto‹ü"?ÚÙ¶-c¼?ï}㌢?'÷ßAæd?ré5'Õ?ƒG^žÓã•?†,0ZT¤?‹3*M&;?ï)¼{Ç?†K-$ü8Ë?‡Ó}ˆDqD?yŸ#'YT?±	Á­†w?}¤×X ŽÙ?ï6ôÄô¢e?"•éc÷?r]c*ð51?aCõ
¸Ä:?"Š›«
?}KÌnÇu­AGN3FGL J1830.0-4439@uâ!€M˜9À.Oó v,­À8ÌÌ#Y¡\À;q¦½n‹?öê—é@Jô@c‰ô5–@&þûɧ¿áun°Ñˆ¿æN­q+«¿êT@([‹8¿ïÿ˜ßé#AGNbcu?ïÍd"zy?uú­ºF»?q—òH\
;?s›z?^×ñº¶(?XµHìîÙO?î» 1/Å7?¢Efø˜¿?†ökžâîG?…¨/:~vÁ?Äuô?Ÿ-ß2ì@¤?ìí²qú?¡º¸]h?°9ë½ùS?šˆEÁý§:? »-^¥*[?'âÊ1‰\W?îk¼Mg€²? ¢"0)ß?"Ø©´JÉ?ü70‰XÛ?ž¯Ì—åè¼?›|ÇÖ?ïç_«óIŸ?c~./óuŸ?aÃNr΄€?`²æùÊ?Kt­An?C°Ù.ÑÞK?ïwÈÕád?~ÈéÛ~Ö?tìÎ9#M?qJ,¹v¿?‡—c{¨×u?‹¸.§?íù2H§Ž¥?•¨§h4'í?¦w4»'?'V½F´ÿ­?"ëN¿—	e?"]+Èv?ïƒèÂ̘Ê?…yN4;R?ðÚphæ¦?yz™2f‹?z)顄u¡?}‰^³¥=AGN3FGL J1830.1+0617@B"}@XGßèˆjÀ8³È
Jk^À;	óžÈ®?ë‡	t¦x®@Éý &¼@â.Ÿ¥¢;¿Ü's'Xi¿Ý·íø@˜÷¿áÁ¼öƒ"¿æ¨GúÀ{AGNfsrq?ïäáõ®ž?i12•
Ë?;äÅ?5ÜerI˜?g¼n¨|?h&ú'ŒÀ?îóïÜtP?¡¹4‡¤­'?u]hm?ubÐSòÊÓ?œ=­ \G? `Í«\@?î?žËP?˜[+J½?" ,(ÿ‡ó?ˆílY¹?¢5ý5Fõ?"HM^ž)?ï@Êۅø'?Ž>ï
ã`?\`X¼Kù'?b6âö4i?– Ÿ£¥}?D^Z§Œ?ïø')˼"?JÅàÂaû?'Î|`xR?!-
»˜.Ç?Io¹â*ðœ?HËULÔÊ?ï©
'–ë?‹ø¾"ªi?aÖ[‹}âX?`ƒ"Rïšd?H彂®¦?ˆñuò¢(Ç?ïW ïr®?ƒò0ª†í–?–a'А?r=W^ܽ?ˆ¡~c‰òp?|âmȃZŸ?ïÌcr,?i¾.Œúá?Róðc¾?Eæ}N!?4?uI
!wb"?h•<Xœ…AGN3FGL J1831.0-2714@]ä ()ÀÑkÕÎ(À9§™¼ÕÀ;1«.íSU¿ØäƒÒï@IA;3²µ@°ãŸø†¿é"çN5ö¿àÔs·þ¿ä¹¸w͎`¿á'.ohAGNbcu?ퟡ2À¹?­ ÛUœW?'¶…ñB¹=?'ŒVo`Pœ?¬ª©Ù¥Í?©Mm.ø(*?êsH•?ÇÁ÷Äû¥±?ž)?¤.y
?Áɑ05õ'?āayW?ëa¼<Ô5?§ã	|®_?¨óªš
€ô?•ÅÞ^)1ü?¸xHË|¾ã?¢×}›õÅ?é²UÐ?°À¦ˆF^?ˆ.»øÃ?'sÉûˆd?Ç´Æó¼G;?¯—M5©4`?ï…%)–c?v–ÛeC?lOû"#Q?'Û;㣃s?•Ù3][˜?˜ïÜ'zñ¢?îjñÃ.ò?¯ØýŠÜ?†‡³Åc?>†sX.™?£½ z|{"?©
X‹–Ój?î‹Ù'ñ?&?'(™'Û?""Y¤2»?'´€oz7?›jKI붑?ˆ¢
'û­?íÅÍ8ÏÌ©?".,à?u:Ÿ™{ý(?cLÀw§Êë?°}ìA–ª$?"˜²"z;AGN3FGL J1833.5-1033@5'° F\¿ìU'?Æ$ÎÀ7Bo§WÈ>À9öáP?óæ¢̙¡@B¤ë1g@#ßâSG¿æɸµ™¿ã"ݧ)hô¿ç>EžMf¿è–¥ôEãPSRPSR?}'4Bï=6?y.«>¨¡e?Âc•m¸7?ÁJE~9kÜ?ë+øS/Ê??ÁŠ€6œY?†Qá0>ä?'q£áe?Ðå‡<ä{¯?Á/îxKɶ?ç3ôÝÌ?¤ÌZ;?°K†\Ã'ò?œGZI)?Í_ñUõœ?¶î¥u×?枒ß »?·ÈXÄ0S×?®ãñ,œy?¤‡¢7'5??È¥üö­"C?±ƒÛ!ÿM5?çèNóOØ?¶ìoòê?€X󍉙?}\݌ɹ?ÁÿzL¼
?ÂmOÜÂ?ë>ÛS^ˆ?ÂÃ@~l¹ß?"w
¾? Að­€?Òԁñl"?¿ëgËþ¡?åõG;—Ÿˆ?ÂkK—Fó?»K±™À…í?¤Ã«¾nÁþ?Ðn¹nÿš³?´Ã­"ê9?ä_-ђH?µèöóäT?´…O±T\Š?ª]
¨<¯?ǯç2mN?©'Gå¿.v?çƒ\=Äú?µü¶É{»OTHER3FGL J1833.6-2103@(UΞ^$yÀÒBß·7À5ü#ü^ŠÐÀ:bÁ'ïV?ÿ,ý|BØ@ ø1T‹È@†Ó8¡²¿ãæ‡Ä–µ¿çWȋA«¿çÍ~d´à¿éZïŠfö¯AGNfsrq?~G?¦¤$:†‰?'Â^qÀÛª?žRÌÙ÷}‡?]'_¿u?›	¢@1Hw?íÏçÂؓf?¾ÛQŠaBe?ŒïMod:?®=íj^ë?«Å°
Œ'?¸ãM‰7Ü?çëMNÙy?²×Ëíº¬?¸àÅ}"%?¦nW	qÛÊ?Ãâi+½ž?­à›1…oQ?ï΀Ì̪q?ƒ½@ï/·v?$08¬ï·³?69¢'"ÿ?xµVÎ?ƒ³ôüþ+1?ïX`¹Ô!«?™ÀÀŸå0? <Ú?…ȓU}x?ˆÇP@r&‡?–:|ÉAa{?ïhŸÚ.ê?ž±×òÓn=?kì~ÌÄSS?u‹  '˜«?ŽÜé³4
Ï?š?ˍ3ç?êØ,+N"À?­i	,DC¶?±ÖÀBóÄ?¢Ƥ¥Í?·gގ$Í=?§3ªYé$?ï÷m©óü3?ceÇzÀu?"×K*?%Êì?í?O–ÜÓ8¢b?cX÷AÝFuAGN3FGL J1833.9-0711@8‰¡_`¸§?âðÐ $ž×À7øUŽU™À9¦''ØÛ?ÍÂkä™@¡eç»eœ@ÙþÀ9ì`¿ÐÁaߙ¿äŽ8ýÍu¿¿æ†BCÇU¿ÚõâûbatOTHERspp?šyZFããA?›ƒq'~?gG´m?oââÅ}ê9?ïíz
ځ?}¨B	‰?ÄQZµÈ?ÍßÎ/+g?¦fO¦ÌÙ?Í|OO×*?é…Vëìo!?Íb×Gœn-?ĝàG J?­[¬à.œ?»&TŽ³È«?¦ââÜ?çs½\Atj?²è,.N?Ù9pE?ÊɊœ•fH?ef™0wõæ?f`ùY8¦ž?ã`üÝ¿@ü?ÊÉ-÷Æ0ã?¦Ññ¹ï?°aHfÃ{?~yžäF?ó·Æöâ?îVÊíØÚ?²¿ø.£¢?Ó}lRõ¬{?ÖI¨0œf9?®3Y¢S?£ÿw8ˆ?äXv¥4½?ÔÔÄz:P*?Ég6/'èö?°ù³h?¾ÞoïHš?¥Ë³¶ÿ?åÊdv2r?±þ!Ùn›¿?ÜûÔÍ![?Äù*fÂ?psÏÙ½8??cWH¸Tj?áҚvZǙ?Äñð.OTHER3FGL J1834.5-0841@7HT`ªdÿÌïû_ :ÍÀ7]öÌz—vÀ9ئ²†Ði¿Û'ÝèÍx@-Ì^'Ýh@]é jƒ¬¿ÐP´ƒ)댿á¶`]Õ¿à'¿zÔ²t¿æOó]ZNOTHERsnr?©ûšU¯?˜¨sã7Ùq?Ë˜Uˆÿ?'"!B`q?îŒS`'Õ;?¡æ©\y5s?·—Õi~sÎ?ÀÉÇYË_?´JªÜ:"?®mÖ ŸÃ
?êƒÄ}å"?ÄJÐÞªE?·£ElÃ?£4†PƒÔu?­¶ÂUlÇh?™jâ}âN¬?ëAŸz.Da?¨3¬öZÊ-?ÍÿòؾâB?¢^S?…઎Ú.ý?ƒ?Š'n˜?è(€Ÿ¢#?ÂÔ–¶Õ?°œC P3?¯ú¥ÎÎ]?œ·[D ù?¤˜ÇÅM"?í¼Åm²á?¶¡Œçù[É?Ƕ™.º¨ˆ?͕
wÁòB?¹"ðë-?¬@8óD8r?æîÉ3óø?ί¢\-IÝ?À¢),–ƒ\?¨.¢ªºS?µ±ë½™LD?  ztÀeC?é!8=w1?®Ýžèfp?Ñî^NßY?ÄäYˆ~á?{хæ?w²Ó{	…?æÒ®†Ï?ÄùτOTHER3FGL J1834.6-0659@8ÍtŸå
5?àºÇà˜ÿÀ7Ã6ù'PöÀ9ˆ2芘u?"2ÛçYz@IŸæ姺@cߣê¿ë.°:Ê?ÓN˜~çf¬¿ÝV¦?oV¥¿à­èÛ÷OTHERspp?²'æëޕ?²]pyöÍ8?§—p)˺Û?­{þ˜À¹k?ìB–À¡E`?¼4‹€"ÓB?Ð].ð¿q?Ñ×Lã2"Ó?´ÒÓ«*"?µ¿òËÜYT?å7(
]?Ñ𪔋	U?ļƒ>
É?ªæ=*#Î?ÇI%Û(R?²àN‡Ùr?å
LçEÙ?¶†õ©Å?Њ,þ:Ù?Ë3SE­/?•"k&ùñ?'Ïg‹ôMA?çÖìT?ÌN²d/™:?§Ã`H»?® ÐzÄPÙ?¬Píbeó?´%‡/"ÿA?ì¾É߇?¾+	K¶À?֟ אö?ÒÍMʧó=?¶ÍËË\?²éhGM?áÖÌú]îb?Ñ´Twô?ÃêÛž?«ÎÎæÂ@?ȊÓ:§?±­"1n¹¦?äâÉ«QŸQ?µñÛoÀ?Ëm¿ÌV¼?ÇÊ}"{¼?9Èò¤W ?'\ ´ˆº?è¢ÁÅv†?È,d½øQOTHER3FGL J1835.4+1349@EÇç@™Å@#}1(ùÀ9ÍMüUyÀ;@'¿aª?¿Çâþx§—Å@Ä¿6@¯r_Ãßé?Õ	j¤Zp¿ë'_º6'¿à { ŠN£¿í¨Î¥êà´AGNbcu?ëÒÌk(?¼"G×ýNí?©º…ˆ=ò?ª)˜ÙýÅ?ºÄYÝR<I?¸ŸŒµ¡J?ëì'Á¢?¸-°‰Âƒ? ™æ«Ò?¥1bRÏh…?¸Rȓ›ív?¾®™V¹Ü@?è(Í°ÖI?­ûh æ/˜?ÀÄ/q¬?£qIx¬Õ…?½13œÃ"]?¥VÕh¢?ç†,H®´?µ¶Ÿ:4²¤? çó$íy?"׺ù}?Íà"â?µc`¶±Ôå?í²´Öý?¸@gÖ¥?Ç`Gx¨?ŸÚÉãÙñ³?¥ñš»·ä?µÔôÌ`ºW?î—ýzi¨?«zžçG?‹	©®'?'iÃAL?Ÿ{{Ö¢ÿî?¤Ãò°!¡?ë3ÔÍïƒþ?¥ìÿÂúXO?¹¨ßi©ß.?¡Y‰˜¡uQ?©pôHŒ—Æ?–"¼˜ª¹Û?ìãò0±T?œ#TîÄÄ@?'Ž…"×?|Gd'þ±S?´ÖŠÞ\§?šÚìИAGN3FGL J1835.7-3258?øß}ž¼C=À&¾S‹'À9áB'[sÀ;¨±gìxd?øN{ÞÓ@ñæ"©r?ð2^צÅ|¿Ñ×Öì
¶¿Ý•»~ã¿éœolŸe‹¿ïÿ\×qk}OTHERglc?"¸ —{ƒ?œE‡Ò$ƒ ?ç/u´6š?͖|¨È?ÐUŠŽÂX³?ÌÏÇ«ER?˜='x î?¬nÊ½Jp?é‹5{•€8?­»±é¾í?ÆÐn;¿@?ÀÁ>ȵ?ÄÌâåE!?°íÁÕq
?æ}šØ]ú‡?´ÿ3áGÇÚ?Á<±¹BxÃ?¨ÍÙ؝?¹÷ž~þJ?®šan£Ú?鑝$Eß?¼N=i†Æ?¹{x^oþ¿?´ü`Ë2H?¢¦ZYS2¡?©ÝÀiUóÁ?éÆ	&øÅØ?Ƭ¢¦Ä¶?Ä>DÍÿ¹?ÄŽ
kÅÃ?·­æËÚ?¸¾:Â+…«?ç.pTjª?¦©
à?Çq7Ì[I
?¹QïýLž?Ôi–òuS?²6÷ÈU?â¼2N‰c?³;fwè?ºÇ8
b"?¡Ž•Âe
ø?͜,ÆÝt?±Ï/Ɵ¿¬?ælô_Ÿ?´­ÐZ¼]@?±gÎl7 ?¥tPðï}PSR3FGL J1836.2+5925@V8tÿñ½G@8ÿ'¿°"˜À5<³»ƒÏ-À:YÌÅ@'@ oa6Ò@Րà?õ:€nû5k¿¿NšlÓ=¿Ûʬ"y
¿æ*Ü#,¿î¨Hî}ÃóPSRPSR?N"ö°VÞ?PéêµÛ	¢?îêTÙ?¯Þ*±ô8?¦¶¯ë+?¯¼"¥­Ö?p*S>'#?¨×ß²Oˆ?ï;`l½?¬+¶"Ê?"‰]®©B¦?š¾î[Ë[?£ÍgùÏ¿d?œü"êBÐö?ìž~°µ?§˜O…îÍ?µ´Xl¶0?¢'#×µ.>âN©‹wVß>óû¢?õ
?ïíõHch}?f
vˆ=î?aøhÜãE_?f?@—?#…Ï)è,ý?3 øÞL È?î'>Xw²¶?ºdfûҖ?¦Ø"¨¯fS?ºbBéDä?e7šÚ
Ù?'ûu€øE?ï
ÄÞ6?ž%"ÿRhÕ?œ‹Äƒwû?œ@ÊpJ?¥XFp°Iè?›©ø<ÚT?ë¬ñU^–?¦`Ó«=yì?·ìR 6À×?£+ÃKpv>çk€è}¤°>å¬ÍŽ+äb?ïí@,7bå?\ˆVŠ­î?b¨h>UÆ?\w;…›®PSR3FGL J1836.3+3137@N/sßË­@0É'àÙìÀ9_Ñöy}À;t.QZ¿³ˆœ•N;@Upõ¶@ÅxÀ01K¿è"¼R"®ù¿á†¢®7­¹¿æοë+¿äÅ4
^ôAGNbll?ïø Jì@
?I¶‰Ë…?@*ζÛ6Ô?CÝÉ÷œ†?:¨Ñ,…?9¬ô®›^?ï"{©ˆhÞ?'ñW*:9'?tú ý1Šº?'Êøä¬ß?"cÅ.Ã@î?²J^€»h?ï&€Êb0Ä?'Öêv±ô?‡åLì"?y闃øÇ?Žz€~ßfÕ?x‰Ë<D"?ï
éÂ?ÄÖ?ˆÊÆ!ìË?i÷™©Z¿?a~­W®?›h¿&Þö?‡ß:b§j?ïý7>8S?/ªÏ$ׂ?&ÁÂóÍ?#ßãªñT®? jÉÃ`‰f?!>ó?ïÕcÔ桵?sMã¤[ê¹?^0wMà¤Ã?T	ëgGÝ?kƒï>3èË?oë$Mª"Q?ï¥Ibõm«?pãv¹‡?v»ZO%?kô­íˆ¶ø?w?"@G™v?^¿"äŠD?ïÇQ8_u?gº{ÃM{?OT¦…RÞ?<7…\?xlán1Ci?fqFš]€AGN3FGL J1836.5-0655e@9áj("?Ád]?Ô´ÖÀ6ñÖ³Ö\À9K~Íey¿õ«µPy@l«…Th7?ÿv
`:Ó;?ïŸíp±C¿ã2dkºc>¿ä5»wà¿ÐÞC\vyOTHERPWN?"kM['T?™ó›h‡Æ?"áNy;©?¥a[Á?šÎÖp?®¯µdÑ:ñ?É?7•=?ÐÙ3¸i>?¨V°AÏùÀ?§oG<}Õ[?è*ÇÅÞ5?Ïӊ´¬øû?¶CN3×­W?¢¿"ö<AV?¸¸èAnöˆ?¦Nw!)?ê y1;®¤?ªG½Ì_?Î;ÖÎ`ÿ'?È1.mž
?Da­lۍq?QD^w?èkñàØrr?È6?óòå?ƒGaýAÒè?†|§6& ?"g>‹Rš\?«†Q\?糖äñ?®
bõ/ÑÜ?ÔÅ1'·<?Õ§«vwê?®æËþ%?¤â']ì.?äžú'¾ð?Ԏ}óuÙ?½'†5A]÷?§qx›Ð´?¼ÍûXüF?¥îÌÐùcK?è¶Ùì´¸?¯nÔ8ÅÒ?Ά(Bšž?È)T«0£j?.åFÐð?1Ç%9°B?è\•Ê­é?È+OŠ½ïËOTHER3FGL J1837.9-0607@9ò€Æ^?ÈÎ_âáÀ7à~SÂõ³À9‡¨ÖM?óêy¶O\ß@ô.·x|¾@"BÀCý[¿ìNùõœF¿×Tj*Kâ¿çfjÆÙ~ó¿çYG·y©dPSRPSR?ƒ®³Pé‰?ƒ×cìF	Y?È7‡*×,?ÇÅô^"¾q?é£chÉÜÇ?È!K±ŒÞ?§GûÕ'?µzÍ×ô÷?ÄôÌ¥àyÓ?¼'͏ÀQê?éQØVæ
2?´0F¢Yd?´£@ÆË? (È©°?Ê\7/äkœ?³Kàð"·?æäýËûÊ?µ}dl¬Ÿ²?°!èÖ?R«?²Sªû…k?¸Õ€xhúô?°ö^Þ?êáÖºü?¾LŒösj?q:ñ9?s-Ókª?ÁIÐ×QË?Âómïáhª?ë‹YTQˆU?Ã1·™E%?²—À?¸pDV^@?ȐJqþ?ºâ¾³{åK?ç·é
ž/?ÄÛ…{ï)?¼Õ*‹¼.?¤-h»ûû?ÌX~'x&?±¹ŒE5N?åfeº™ïU?²O<	bا?­{ëmE?³ÖfÎr¶?¾™Ù
s?«ú7Ð0?ê[m;]?½û¯°©¢ôOTHER3FGL J1838.5-6006@tõýç!À5½v Í|À:$Âî&¹¨À;¨¶urrä?íuúÅn@2E³"k?ý´Ü€žöÑ¿â6wM‹Æ¿Ô€[j3ûZ¿Ø3Tq­}¿â€åC!ÆAGNbcu?ï†1Apí?ŒÍ"ð?\·OúI É?Zê'ãåV?ŠÜÅÏhÄ¡?‹³pÍuÿ?íã0Û•p?±[Á0‡=i?–Šn|Œ!õ? D¨ÁÏÆ?¦‡À¤Ü?ª|Ë8À>^?ìíÃ}vUû?¥'ü"üÜ?¡õÞVì.?'£øzø?¯-駋æ!?ŸëDóT>ÿ?ël¬y+v?©Žª°ËÂê?¦—={5?¡Lp{P?¹PSݓ<µ?¡§ãÔé5?ï½åQÑs?~­Ô-yñ?Væ˜Ärr?X=|Æ¥Å?{S";Ò%?{Xïdb9`?ïL'çgœ‹?šïqËH?|´T8Bÿ?'E.
ª?Ž8&º?•cngÑEc?îÍ©¦#?'W†ÁÔ	þ?Ë
ĉ"Y?ý±õo©?•½s•-a?ˆWÚP{À?óÓ;?<bÝí?¡È–0¼?‰Ä‹Rœ¢?šê>š-?›zn¬îAGN3FGL J1838.8+4802@S<b?û˜'@5ÔC@ÇplÀ8öïÕ'À;BL¨O??ԟ|EºŽ@¤%D24?üåâDhæ¿ãEÑøGq¿ØýÁ†óyµ¿×bÝÈë0¿ÖŽ¥nRÝ·AGNbll?ïùÀM|€??ù'îÛxh?21Ö5UÓ?-u¬š??̅r<º?6úÎe]K?ï‰ÜTÕw?"šs?Zy?u&º(ÿ?sHD‡Õà?'õp€´?'Ì<£Hì?ïkõŠ8Ü?}TŽ•ß?"üù4Z?t@åiûî
?…qê늗?såBñ¶uü?î"Ó*E4#?"@ÆLdŽ?pˆÑŸî;?m)¨'¢]ò?«Á³%G<t?"˜†ËÀñ?ïüaØ뜤?/-(À"T?*Œg,•Ú,?"AúMï?/V
‰;ÜÕ?#WÚƜ·Ã?ïÓüä›º?x4õÿA?a1)Ct?ZC³"?jÒ9,Q‡?t*º"'"?ï±Ì‰cŸ?qÜÍøe<?r³}æ+4?lR_d'¿y?tf¹Ùé2?b>~ùÙÂù?ïvê|$¬?sr⺻£h?dÊJÓl/õ?R=ÌÙªÞ?ÎJ£?r0oŸ GmAGN3FGL J1838.9-0537@:€o_3l>?Êxßl>À6ŽãðÕÀ'À9>áÃÔև@¦`Ž@
Ì]ÓG?ÿ}³Áä¿Ò˜b0Œ¿åÈmÈì~ª¿ã…j²SŽ¿ìІ^1PSRPSR?HÀ"@CÓ?Nf¾ŒÆÒo?ƂÑÝi
q?ǖ:âî¼?êY€ÄE?ǟ,ºŒó?b'€Àß?<"Sî±?éêé‰à­Ä?·€º/fJ?ÈQm…êe9?·€Ðâëy	? žNùÒ[?—Ӎ2†?Ýõ–ðqî?»ñ0{À75?ào Dê¦ä?»ÕàvÂ4?L"—ð"Bš?Rn_©€?ÞH3{閘?Åáêÿpk«?àÔݜ»G?ÅóŽ7eÇÛ?ÌcÂïþ6?*€W±x?ǐE	@èË?ɛëRÖí?êðZµG?ɝ¥
»@?2{W[—Rø?U—MP2<?êz]¼ý)•?«!'|î?Æ
K`.F˜?«9äÎrt?¢0í]»òà?™é<úDDÍ?ßsœyÙò?¸ܯBù$?ÞFƷΧ²?·À7ªE¡:?AÖØðÕMà?EòwŸÃË|?ß(£·ŸM?Áh7ÆY¯ã?àg8nx?Áuˆ6£^MIXED3FGL J1840.1-0412@;å`Ÿ}i?â£t?ܨ§À7«À_AÀ9Íúꉯ?õ{*ˆ"¹‹@?­le@Sõ?ݐ"¿âgrÕàqÅ¿èƒÝRu¿æß0$˜;¿ë"Ï"gˆûOTHERspp?`‰oEðu?aô1²?áA«dû¶?ÑÙøÒ¸ª?Ý\³Ë°(c?ÑØÛ\÷@®?Rp@•?j3íø~r?á»o4ô²?ÄiOë¶Ù?Ýê9'G?ÄjÜHQ
Ë?²Ýãxs?›ÛïÍLÌ?ÛX¨{g]?¸¨Fæ!?ßïÞ§73j?·ñí³®5?"~·Œá³?"iRf˜¨?ÓΈóx'?Á¹ów9%?åÆÁ#»	ñ?ÂQ¬+ÜA?@c¯Áû?C·åf]¨ö?âÊè·öG?Ñà~òûH?Úb ޔAã?ÑÞàíãj@?}\ºÔmA?™C2ª<?á[
ê·ï?À[:ñÄ?ÜÔw@~J^?ÀWœê1¼?¸t©`#:É?¡Öûš'²?Úۜ&wÔ?´H`õÙÎw?ß9€æU›?µ	'؍´Ú?‰üÙr3Ÿ?ú.AÍMþ?ÓbfÝ.ĺ?¼Ñ€XÞq?åæÙ+¼µ?¿¿â¿¹zMIXED3FGL J1840.9-0532e@:ËÂ@ÐO¿Ékd'õµÀ6¦rKPÀ9FS£C^?†è×sñ@ÙÀ»¡V?ü㪟PgÌ?ÖzwéDR¿½EÁ\\¿ÜàÝÓNq¿ßϓ¼
êOTHERPWN?YD×ÚÎÁ?¡ÇÃÂoÎ/?t´'d?ƒ	*µY?îípØãº?¤"]þ
?ËV1
ËX?ʾéäy€Ž?¯k{gïh?©Hÿ¡µ?ç3¼ÎGÄ?Ëü‹6)‡¹?Äü¾¿Ìg?¯­¶©lAê? 3Íõ²B_?'qG¸GÑó?é½»1e ?°£eÄV»á?Ɩ­¦¹4?'i‡¶ Ä?w'∲Sí?zö"R:?ê+YéA£?ÂÏlÚ
?¨mñš¨?¯ÄÊc«?‡i+×c–?¥mFRù?î‰a¤F?³Ä¸s|ãü?Õd9ÿ?ÒøÃu¶?³¥»ëòå?«UÕöFaÇ?âÙ+ÿ"?њ'áL>P?ǦÉ
©ø?°D#ԅ"Ë?©é)%†?œ]'Sð…?脿*Þâ	?²¯£ÌAo^?Ãջϵ›"?¾ƒm˜cu?peÍG?hø‰îµx?êéŽAªLù?¾ª:YJҕOTHER3FGL J1841.2+2910@M8"€,á
@-É0ŸÚü:À9ØÏL
ÑÀ;`,ÖøŸ¹¿íό‰Š@
Ž¨'ƒ?ùóÀ+©§¿ê2þÄZ|<¿áÖ©Ôò'‹¿ãijù—03?×ûîwUnAGNbcu?îy²s…3?¶õZ°¸‹?aݯyÆÈ?f¡ê~ï?¦Ê‰æôf?¶ËßÚã¿?ï'âÏSËë?'z3Ãø@?n½ÄóÄÆ4?nW§"€–n?‡—Úå"ͱ?{NŠ9šÏ?íÐJR´'Ô?˜¡ÿ&É²?•?"sµÌ?"ÊRê ¬º?¨[˜•ÂÝ?"Š÷•MY¥?ïCJӖs'?™í™¹¦–?)F ñ1?,ÇóÆÁ"?—|xP½•?™éaYÁzO?í¯«3z7?ÌÝçb‹v§?P…j'‡?mà?"õÿ"?²BdPú?ÌÖK6ñ??ï×Æê¤gî?ußs¨LE?ZrÊaÛ¨?Vg¦¯»Ë?jÿ°(l$Õ?q¢kikj?ï%Y4Ø-?‰ªÕ,ý#?ƒyF«]?w{6ÅÍsÎ?'ŸÍ1ÃéÇ?…
kÓ]–¦?ïà#]ÖA?fˆ¤ebÍÛ>÷'©˜ô¯?ä³Å"¢?o®°Pw¶?f""%HÓEAGN3FGL J1841.7+3218@N¾'?ßéà@/úÖ 2¥oÀ9J±ÓLBÏÀ;i»Þh¿ðôFn#t#@¿nëE3@v>ËLo?ÑÑ£=S¿è¿èiÜ̳¿Ý9"ûƒƒ¿ÈYÀÛÒÏAGNbll?ïÖõ´fhY?zaÍ)"'?QJÛ?8{?P"ƒó,]?p2oÇõp?wãāÂìÞ?ïovxŠÞÉ?šdpG.Ël?qÎÂÉPY÷?øM'·yW?‹;ç¢?—•a¿{?î©õ'œWî?"×ñ‡†?Œƒ†.?€öÅÎé£?œÇ 
B?±gõi³?ï
/ÇG?'ˆ²àuGÁ?(;0gÿùW?/ͶžÕ?ž)±¹W?''C}†•?ïñ'É,?‡÷xô°?BjÕÓÂ?gŠ¨4D?T½¥té•ì?'¸ã*ñ?ïÔáLqÙÈ?t–Yma†È?[äªw¬ò?TÁãz3?m^Ádåa?r*ᴟ1D?ïzö›ŒA?{á
Cýù?|߄¶Øå?m¯miX"Ý?'Ò¹~Æïe?ugt_û¡¢?ïÓ`‹Â'?e†±^Ù"?
ºFZ?xE_I?v=QÙ?er~µ+2@AGN3FGL J1842.3-5841@u?«ºÀ5Ë{_ò®ßÀ9È*"yÀ;~¾|§ñ?ÒCP@y¿@
»?ÏM?û ÷ÿ«q]?îÓ
;°bç¿ãÔÃRis%¿Æ[h…`¿Ý
7+÷eäAGNbcu?ïðqDw?WD'ðyð?+¡ˆÜ}æ³?' Eã°ø¢?\‹Áùaæ²?VÀ#Ë$Ð?ï1d
/r£?›ö‹HYFT?vÙ²»·ý6?xrâÄ[?"O§N?™Á ©ë6Ê?ï	i"?…%¾Öj?†¬ø²]ÿ?tÑïÏÅË]?"ˆƒ`‹õ±?oz'㚬?í9Ø[ÿ¸»?£øR²`'$?gãúl~?gɟݴ³G?µrM\˜÷?£³§Hð?ïùW×yÆb?Pó
ËùNÉ?%thÏCå?1Ö¬Ò+3?ECˆwÞgÂ?JT`ODè?ï¸o©õÌ?É\­~‹?`ɏ<à¼\?Z@)@a3=?{ccW‹R¿?MPs˖?ÞÄq	?nÙ_j½R?wþ
~&€+?cÓk•®â.?€SÃîŪ?cH"'IŸ?ïM	4Ôjr?€g"ÑûY?b»lÀ,1?QöC¨ö'À?"áõF÷2?"bÅ«ƒAGN3FGL J1842.8+6810@X£Óßæ…@9ÕiÀú)À:-¼±Ì–FÀ;¬à‹Ær@¿ðiö¾¸¸@wd/¥µ@jrà_Ý¿ãgŒ"S¿é´µÜ<ε¿ãNtžîî¿âì?œ€²KAGNfsrq?ïþ¹"à>?*JËÅõ\>ð¾Aû>íϟòb7q?,¼¢e«jV?)'È~~.?ï¼÷Æ[Õ¥?{÷7Må‰?l&Ž-®z®?jœ"RˆÚ?spÕÙz€?tr)8kªì?ïsë-f.?uvHßoJ?u,½ö_¶?^â!ÒWº?ˆx©l4"?qvXpµAç?ï¶y¿è?u½­²ñ¨{?(Ä.^|?'ZœeEÚ?'¾UÄt?udò_»ÌÔ?ïÿW¬fJ?]ß7£Kß>鐣®Þá>äÊâpwò?Ø}l«¼"?U;:es@?ïãWDNRb?f˜@VCòá?XXi› •?Tê?`|†º¢r?_{¨A¦E?ﺁ.œS?jÉ&H?ê?hyÁÑ]ã…?LÿL9â?v·^p4°¶?h.ïF<W?ïó¨½Ûæ?L.ÎC˜qü?
®Hrø½?ììÈýïÚ?WÚ~àñ?KÇÆ
È83AGN3FGL J1843.6-1114@6
€_5ð}À,ß?ëþ@À8¥
¿cíÀ:š`' ×?ò— rç(C@DO‰€ï@ϔÀkëa¿áyÁùCñ¿êi¢'¿ìþ]YÙe¿ïÿzö…ÍPSRPSR?§§-ލÿ?±jÀZ|?¹5ۍ$®E?ÁÎ'ãZý?ë^Ñ°rŠG?Ɵ'3@A?'nÅåºÊæ?˜¶¹GÜMù?ã'wåGu"?Ä03×ü^h?ØIš'Ôd?Ä]ÂË8šs?ǦóQ¶?©æãíXf&?ÑxC`Ûj¨?±•PkŸ­§?áZWÕv??³ãxŸsÚ5?ÅTsÏÏn?"×pa3n?âþ³!ÑÈ?Á{-GáÀû?Ø&D"ÑÖ?ÁTâãî3?®¶?›
-?µ¹Ä
]0p?½i¶R[?ȧ`Ü?êrmÑrV'?ɘùi@"?¤ÛÞN·þ?³Æˆ)`ŸÉ?âñÊñ¼'?À°ü›¶C7?ׂ~Ÿî~?Á"•ÆÑ¿?Ú
†6††?²ú¸tN|'?Ì­'Ú©H'?«{aðìÚ?מåۈô¨?²‰ä²×	:?°•òòh?œ"yce?àpÆ=ÞÕ/?·šÀÙK À?ێץˆ?¸/6;ø¿õMIXED3FGL J1844.1+5709@U­aÿÏX˜@7z—¿¤ÆÀ9»J>³‡À;ÃhEc·_?Â%¿Í_ïª@Ó¤'UÛ@\ 'F¿¿áê£Åê0¿ã3xV¿ãµÝúòz¿ïýÎ xµ7AGNbll?î¢$ÇNwv? —rr˜Œ?¢ñ†=çÚ?Ÿ6r'ƒœ?zf¦ú8?tTñëZ!?ëþ­6¦ÒŠ?·èÅnè¿?³ª§öv
ì?¬OU°d ?¨¿Üª^?°<a(¨¯?ì«]Ó^¦?£eîÞë>?±¢BvdcÁ?žœs°Õ4?¢à¼s?ŠÂðÃ¸×?êæ›)‰È?­þŸ®‹¸?·Ï­ÕÔ?©å=·­>?±KW4åÒè?ŸÖ×<½J¤?ï­ylA`Œ?}+ꍩ¬?€ÿ°®lè?zéPëÏ?]¡îZƵ?TrðO˜J?îªjNþ?á?ž¯_ñ°›?™×g¤aÆ/?'Ÿ.ÙÝ+•?ÛNEٟ?"´YöVU?•Ý2²?Ž'@p9w;?ž±iÆ¢y-?ˆ‹°òù?4ñE?sôš0—F^?îʗ:Ä¢?ŒlŠòÖ¯v?–zI¢'?ƒàœ¬V\C?2™ZY'Ã?"‰øÓÅAGN3FGL J1844.3+1547@G&	_ûZ@!RaՈ]À8ºë"ùÀ;µ}û®b?èqP¾ù@'L(!²,@9v7]d¿Ùnÿmš‰¿×¦on*ˆ¿â›®rÕÆ­¿â W·³\AGNbcu?ï¡æºè&x?}æ0°(Õ?s³ܘÇ`?kKO•Yºý?{YˆÎðdi?u¥XE¤?ëýT\û?Æ
ØO{­?«øçM	•?²§2yüž?¹k¡¢T×?À™‡…?í—`Y?¡£â·‰ˆn?¡¬äˆS?ç'…Ä¿Q?¬Òb‡æg?šÔ$S=»?ãPlö3´Ÿ?ª¿l'X?½®-«›
?§{·'?Ñó¢GÏB?ªäþs…?ïäDóhÝ?còòß&?["¡"ck?U‡ñÀêó×?[òSÊ 'Ô?XãV(ç?í›w™ƒc?¾Úú'Dû!?"jÔªÔº?©sÚâî?§~Ðû¼–¢?³|³Ð³?îá8uxŽB?Š³!Õèª?']Cج?ƒÅæ-5ã%?'{­z–?€Ëmí'kÝ?ê㕱?™qÌ!ád$?±¦³ÃZk?" 1ñç$?½èÕ³|ø?"]{•©sLAGN3FGL J1846.3+0919@DX[_¢'@j!€-aãÀ8l|ÚF2À;$î?
\@üɦ&Ž@Mn=p3?îe@×\?¡þöÉ(0(¿³',²Ä¢¿á±Sißl¸¿ì…0-Å5)PSRPSR?u܋ܗ›?€s+¨È´+?ïrº8ºJƒ?ŸwØl|Ñ?ˆc+êÉ°?š:?ÖŠ?®¬mâ&À?ª7>ü,E_?ê6gdWf?Äÿ:6¡k?Æw©Û?ÄÆ`Ð?¢µ^ɞuö?–"#-.´?êÃ
™a?ª^
rŠÒ?ÀF}è¹"?§"•&ry}?¡2ÎeQ‰?"'*÷U?ìv¾]sM«?¬†©°p©>?³Åó«
(j?§É·ý.Ê?q*җ_(??}œËÌ mÐ?ï[óóí<? Ö[û>û?6ÙW‹x?ž_'àÆÅ?Žr.#\"?±†øWë?êD¯LçÂÐ?ÁYW¦d'?Åê+,?¾_4îÊ"£?©"txf²Ö?œý$Õã¦ø?ê3x-õAò?«Ã‡@à÷¥?Àé'(þjÃ?§{Í+Çx?¬Ù9õG©Þ?–V
"&¿½?ì‡&ځ¸Ÿ?£ä
@'\ã?ª´XdTš4?œ`}òº–PSR3FGL J1848.1-4230@vó¾ýÀ1cŸVqýÀ:)+rt'À;ŠS².»Õ?àAšƒhC¥@
n¦9R?ÿ8ÿ€SLƒ?ï2_zÜ6š¿ã¡[Dý¾¿Ùd¦ÙÚ8¿åb©a§~£AGNbcu?ïï+z
?z`ó?T™íªva?Z-ýˆ'<‰?‰kálÅdÉ?³èu*ì–?í#eÊ+?¾\«o¸}=?‹ØÒÚû?£"zà_Àt?¯º¥¦ïÎ?¸dšVC?îQé™âÜ?'¹rwÝ?'~.q<	D?ZeëÞ?¢"O,°Yœ?‹Í˜='Ìe?çÞ_W)Ã?±ä¢Ò¤é?¦è—zýĉ?šåôH¹C?ÊÌ\Å'çÑ?±Ð'¦Ä?ïÜ7¶_´?'4´Z?³?B#™0é€?M"'W0"?o?û>äe?€§±çƆ¸?ïj»×ÿR?¤€n†b³"?'…äþ>VI?"ùs­À¦?'ï¶TŠ? mÝ#î-?ïQ˜Ào‹?|1utÊwö?€u`؜‰š?hPSÍ/?‹$nÿz³?vÚRø7ô?ìö9Ù¦¶?–¸ª±
~?ŸòøõB?"G}Rž*ö?°Q«u¥x¿?"–,ó@8†AGN3FGL J1848.4+3216@Oˆ M@-[ç^jÀ8&	Ñ:×À:_ÙuQ»´À
˜wDŽ¥@p'º}ý@JÇ?Åí¿éªî
¾à¿Ü&âå4o¿æ´Ô¹]⽿äVžÙZµêAGNFSRQ?ï¾9T=!§?ƒ•ÕÑ@—z?`ïGýïP?l2×þºÎ?xk²'`˜?€ŠôÖý5t?ï"zPÔ?—>½Á?i‹Õ™Î•s?nL	Ú?€?"جÕ?•pk'Aÿ£?é鼂ãÜ?²Ñòuò®/?´Ž"]é–ç?§
Tg»o?ÁQݵʟ?­âã×®¼¼?ïړ½Pê?}#§ÊH‰>¿
µ}EŒ
>Úç!«>€?r´@E¶´°?}"PãÎk:?ïê'
;ÛV?pmS0ÑÉ?TúÖ÷µ?eä´Pþ?ù?U᪣?cŒùàB«º?ïÚMÍ×þs?zÑ~¡"dy?UJCClSu?RÇWV£Ü±?k
'+ÛO?xø¢
êwû?éðÜIu•?±n:?°_['•†•?¢Æ+äX†?ÀáFνà?«KXÇV9?ïô)``?[ôJ±Qa>xKп}>‹œ€Ž"?W­šŒ!–?[òÔÛÓhAGN3FGL J1848.9+4247@RÁð`P@2{_L–²À:i»dgÀ;¹ZúøYC?èéQ×|î@ G"g{d?úV¾|'¿îÃò¯Ø¿ÇJÀ©º	b¿éµ¶¯]Ò?åwÈ/üiAGNbll?ï¯ÊöˆÝà?ƒIãYÎu?téD›X?wuÇD/)?s0÷g'Èñ?x¾áL?¯?Ìät´?•*í/?vR'n'&?'y"9b23?ƒ®Ä}Ý?ÜR7§?íXôqñ"Ü?¢ÿ"Q.'?–ÌÃCŠd?‰!Á]Ä1?¯oÒ~p&?¡¿Ì"ªø?ïºZ?¢¾?¡±¦P˜;#?|MK~€Óî?˜ŽþŸ¨ˆg?—õaÖ¹:?™—Üåz–ë?ïå–#寿?uÛfÃÛmï?U½a3ôf«?`îÍÀúþ?_W''ºñ?rnæñÈÑ?ïفaÖ?vZ,CB['?`Ìלü?fí'%ÊD}?fp,œ@ìó?iùÒ¤à*?†¨Œb?–o¡¾Ô?'¥Lé\?ˆœ™·?žÕ‰ß½?f?"Ï½–?ï×
^0jŠ?~³6ûI?Vŝ°¡ë?rDEÊ"š'?m"ß/wÕ5?tžôF–@äAGN3FGL J1849.2+6705@X_[íöé@9
` ÒŸÀ7¼0íޕLÀ;)ÆΆ
q?øÖ)vò@8t1Bî@ðwy‰-ç¿Þã)ß]¯¿ä Ì=R=\¿ä]ŽGoÄù¿æàS*°"íAGNFSRQ?ï÷ñ˜€ŒO?Gª¹Ñb?@í®2ë?@8‡¢u‡(?>™
7)=?:Þ½5ÌÅ?ïÀ¨Ÿ¤~-?(Ö³_yF?iQAæ·?lQ*¼*‹ï?s&¤OBB?{eو"ø?î–mÒìK˜?šá)_«Ô?šJ>"Îp?•^÷îWš?'è¨ï?î]МŽa?ïùßø×j?W»8užYö>û³𡄠?°$ØQÅ?G¢"µˆw?WzGC‰`G?ïûIóû .?=3ÿ‹¸W?:k…î~Ke?6µž…É"ã?&‰±/'ˆ¼?#H"ƒ -?ïç=ø=
?f›·_¶ø?U'ã¹Ï¢F?TM/'ÓE?[òü,zù?^'nsÉÜ?ïæ;]Ï?'ãô	;bä?'ì»×;x˜?í\?ˆlùv¥®
?‡Ä-é]¬?ïÿJ½,_ž?(ò2áSGP>á5FV9•>é¡{Ÿã?µÖ§¦?(§¥6·øVAGN3FGL J1849.3-1645@1³q¿_üÀÀmœ@ÔÀ9Ö®8HÀ;=Øwûº ?çºõ¬¿ç@
~ Lf?ù°ŠŸ*Ó?åUc¬En¿ï÷Š9™­?ïÿ}'Gÿ"¿Ú	ÞxúE_AGNbcu?íøVŠ?"o?°X±ý""?W›ÝŠ—ð?WíJĒø0?¯½¸rLΐ?°Cm5_Í?ê/¯oM?Ï
FuÁ^k?š®<«çUã?£EJ=p?Ä-y¯]??ËÕ¨¯rZ!?ëÙ}˜ÃA?© Žj?—ÉÕ'ƒN?‡Tðÿ#dž?»Aï"¢å?§ Æ1É!?êqKXì?Åi¯'R£;?dîu¿ûÓ(?€
¼§$Äs?Åè4û=D?ÅYxgŸ?ï$B@±ð?³QÖ«U«?T$ë™?TÖ,'íI?š5oÑÞªQ?NPV?ã×?흈t‹Ë®?Â
¯RàÄô?ZB‡2:š?š­¿2³Æ?®Ðè
kq?¿F¯ÉS=?îKÇ°#?—8YÔ=Í?ƒþžTP?rpŠ˜Q|?¦CýRHÀ?–;z×Ñ?îDNQØËð?°
hâÒ?z§ \õ+?'BÆwhÚD?¨f&Óèð¦?­ 9Š)AGN3FGL J1849.4-0057@?Úý¿³ß–?TÜà‹À7½ð÷3©À9¾Ç¦^Û?ø»òː7@y'W'c?ù'cð?m©?ï	Bi1¿Íƒ'[·¶»¿ãµ3S£K¿â¯ò6á"OTHERsnr?x™âωú?t×w*²Ý?´9O'Á¡1?´­øLŸ™M?íG¢UwM6?µ[ÌJ"?ƒrè!^kè?˜€Ê7=¦K?Êì,™;$ï?ÁïhÉÿ#G?è÷)9+½?ÂláÑQýà?²\`Mö×? ½\©/V?Æ	"-*ä?¬Šï¼ϊ?è21ÔÁì?°'Ûó}ñ?¡&8µêbS?›ßÂ

¡Ã?ÈWÐê¾¥?¸î&nÅC?è×ÛÀth¡?»|¢ŸÊ¹?sèr¾?x÷.²´_{?µ=ՂæÀ?·å–EœÚP?í6o%&Ö?¸"FÌh?"m{A°,?¦
Ü;?ÑÜLÅ^!&?ýIÂ@×·?ænmÅ;š?ÄÁjÆíj?½mNU+3=?¥%S²¼?Ç='me?«E‡SÞÞÏ?惿T¿?±ü¾Ü?¢õ/´¦úÑ? º/Z5¬?Êý|Åòg?²«ëû˜¡?èMÓ¦
y?·"Ëk©OTHER3FGL J1849.4-4312@vx@À1Ú3çüÔÀ9C΋é®À;UÏ2e®?꬝ØB¢@ê#3
ïG@"›€y
¿Ñ¨õRäÄ¿á9£ª¥}¿áҜH[ʒ¿æ—þ7d+ŠAGNbll?ïêqS\üä?^­é"z;?QDх_ ?PÊÕ±aß1?Z	ëz?Rœl袟‰?íW•¹ÌP6?¹;Ȗdäd?™Öýð^¶ê?›êÖmÍrk?­›%lÃo"?µa§ 4Â?î°Ùåö$Æ?'^*îñ.?"²°–á.?ˆ´_¾b™?–W™;Œ?†
­¢?ê¡ñ+ü³?£™o¡OOÜ?¥Øë(­s@?ï2õ˜?‡=r7'"?¢S‹-Ë3R?ïõ¤=GÅM?R{?Bg@¶Mó?F3j•¾üQ?GÉT6[?AŠQ±?ï%…5"?¢–LVF'ô?ƒÄàÅ'<?ƒX¨PS¶?"xí§Î	?b4)\­›?ïuÊN§u?'=]ªg^"?'×»"3fI?|¼ïur'?kb_×½'?n7üƒ7DG?íÏmÀÅ$?‰Û2§XZE?›Èìjhb?uñ뮦ÿX?¥$­¾§‹™?‡ÚûÂ6NyAGN3FGL J1849.5+2751@LøÌ?ß @)a ˆ5ÄÀ9µ§íÀ;~¬ 7?ñ5†oE],@ãîƒ*í?@¨8ßðk
?Á—'ӝeE¿äši¿ê!Û®"N¿ë.¿±qAGNbll?¾©râmx?º?Aç߀a?ëÕçC¤"?»BÓþß|?…s¯3»—'?ˆ×IŸÓ'Ú?á&rQùiZ?Ð&"ÚãU?ÑíÒg&¼?ÃÐ	$8eï?É&[L
?Å0 Ë€á+?âœK‹ÕÈ?¹GI#Ï+æ?ÕÖÇ1­L)?·Êÿy§ž°?·¨ßÖ?œ½ ü1»Ð?Õ×HIM"v?²ç•QÀ¥?ßG>
N??¸6?âV~?ÅÃLñJZ—?¯õϊÎAð?ÑûX<¿h?É<æBó"U?楾8ø?ɛÒ2V-M?‡Tû	pù?" h=%¯?éýkG™?Ç#~¡èêÝ?¿Ã0Ž4­ÿ?¼IðN‡!?·Dä1ã?º?h ñl?é±½/~{d?¯,£zY?Ã^yùÒOª?«HÚéq?§jE;V"?ùUPpY$?äÿa×áRì?¨¼r(݁?ÑôÍÇɃ?¦?Å{•d»?³•°?œ–õ5ð¯MIXED3FGL J1852.4+4856@S¦ó?þÑ@3õà_PÈÀ8†oÔ¤1£À;Œ.î¿¿ë$ồ¶Î@˜qB7ˆ@|yÿËQÍ¿â?J«k‡¿å¯uˆ8¿ã‡fýŸ¿á¤mÇr‰¤AGNfsrq?ïï§õŸKW?i×CÊð? =
a¶Æm?7zþ`»Ý?^¨sf©?gÛþ%"ÓË?ï°Âêd§
?‹Œ4Oi©û?jKšÿ?kJmš4?zx"«?Ï?‰yT"î¡Ç?îaójùћ?ž'‡_+õ×?~ܒÀöû?qàÍ'?¦6öŒ8Þ?ž/ÑA
=D?ïõ,ώ?–?[8'AX^j>í"ÝØðdt?½Ío[íN?UkVÒ×ù0?[&‹ptÿ?ïò'!#ˆ"?AEŽH"?=ê!%?|xó/V{?T7;8aܙ?'aûDDؖ?ïã>9"?jÇoԚê±?V…lôô?S+¤ð¤@?a³¯dÈÍ?ehU榼'?ï\8\Š;û?ˆ3òú¶ü?rý…q¯rÜ?kTT:ö¾;?s&²-Þ?†–ãôÁ|?ïþ'ÄŸ=?/E!yô£>¿waøÒ>Â*UbCä?&¤ÊóÐu?//IÆ'ïAGN3FGL J1853.2+0006@@€ŸÍA¿Ö!Ÿ¯T¹À7¨R$AÀ9í
ÒÁÙT?þ™ ÍÕá@56B²,@6L,ÔIn¿ápòÁ~%¿çr(+mA!¿êˆyê/g¿ã­_cŠ5pPSRpsr?vå@óxzÁ?tä$ôShü?±¢½cž?·¤âL?íÝÑàe?·¤ùú {?‡åïÕó$?'§®Cð{Æ?Êï4
ž"€?ÂÃ<$­ù?èä›A~>c?Ã
;,%ù?²éÇè'ò?¡ÃýÈҞ?ÃE³Fq‡?¬¶¶Ñf?èцHۀ?²¥ºÞ9'?£'Ù0êJå? .Å?ƒ±?ËP¡å¢?ÁùÃeoñU?çòª- Û©?Â@‡JÄ2?qö‹·¬ž?w|ž…=v?Àšåz~Ýg?ÄÖv—"L?ë·(´Q-?Äÿ³.ô"?˜´†ÍªÈ?¤ºš¨â?ÐΚE¢?Ãäûú"7?ç,ôyÜ\Y?Äùa7IåŸ?ÀÞï¼2m2?¨÷|j2™?È1¸gm«?¯´Lo¼Í?åÂ7£bù¨?´7¿^&(?¥¦]à Š¼? Ò¡s¾ÏÅ?ÓéP©öÅ?½Åô@?ä°òÄxÒ?Àp,«ã%ÝOTHER3FGL J1855.1-6008@tþí )À7½F@V1eÀ:Îç·3ÞTÀ;úŒ3‰M?çv1Npj:@›Â[YÂê?ý'(º3?îÀšdoÁ¿ÔÜ	
•°+¿ÂÜú.&Pn¿ß
ZO4y7AGNbcu?ïî•$¯?[ß
 Å˜]?Bør*?FÁÚûZ?ZE¿HF#?VÜ×1Ü¥?î²VÈ?²`¹µãZ?"ã†"'Œ?š´½UnC?¥CŽ´Z²?­íßòèl?î|ڝ´ ?6ÂbOPV?'²ÆÂR¾?…|Þ:ü?ÌTî3?†fiˆÌñ?ëêaXh)"?±¾àKÀÙá?¡À*}Ý"?£®'*‡»?·Ìßü†L+?¬l­©ü%F?ïõ° ?KÚä4û,?3s‰ú?1X­VN¢«?O…þ'}ÜÉ?G4*åhó\?ïPe¹uàŠ?ž$,p{‡?{‰#ƒ&‹f?"ê}'yÑÚ?Ž!ÿØ]'»?—vý90‹?ïHŒ‡•ê?€&\–†?ƒÂƒžJÍ?w!ßLxøé?Š8YÂüÚÖ?sÏ[×Èý€?åy¹L?•æ­|-*¹?˜âo֔±?ÖÅÃúæ?"©;âªÑ?†Š¸™þ³AGN3FGL J1855.1-2243@)½«ÓÚÞÀ%ÙHßlâÀ:IR}ÔAÀ;ˆÙÔLg?ðÖ{<6g@.ÝTYs?ý"ÔÁ7î.¿áøK€±ì!?é€à¶cª¿»-""Ñ¿ä¥wžG(^OTHERglc?ï¥iZ{ek?ƒ²"³ä¼?p•<rúÚ?qúÉì'óç?|¶§Š;¹?|ëVQÒ¤ã?çtËϪU\?Î+ÿÚ@S?·Z"åÉ ?·@¯\·V'?Æ¥£yR}?Nj4š#ñ?ì•ÔTDi«?£Ÿ4ã1t4?«lÚ¤Ãó?™š!ºöò¡?«6©Ý¥_?—GUx.DI?ë'ÌÓz2n?·d<'å?º	áçLf?µÏ蔌;#?¢Ïný3¨ì?¡ÃÎs?ï˱;Ì´Ï?zü<pX‹'?g°Î	Oï]?h	;ˏ£?löUöAf?rñ·šºñ£?ì>—)ýªe?¾˜˜#)?¥¦]ûLÒ?¥S°Á©X)?³8#§î?µ®Þ¾"ƒh?îc؜䧵?–ÏyOjü?Þ7æóªâ?Wêy?_?•¦´u˜&‹?‡
èëV?í&M‹gì?¢'yÑ;"?´r¶WŸ·? ªë®<Ók?ˆ"Öô·Û ?»	2.''AGN3FGL J1855.9+0121e@AS°
kù¿ØÙ"`}ZÀ5XôÀ0ÝÀ92ÛŸ'@¬	íI@Ö|O[ÝÌ?üNoVÏðn¿Á~õÔX¿â*ªcy¿æ;êý9|#¿ëvO²ÅºŠOTHERSNR?˜¦*{É?Ÿ¬çæ>ôï?êŸùL)Î?ÈJ'b'E?€»;2?Ç\ðl My?a°yͳ<?/݂ˆA?燡Ïjƒ?Ä¥‡Ÿ­@?ÐÎr†Qµ¢?øÍy΀µ?ª
|/õh?¢í®£#؎?ã"ÃÓÒ®?¿+Súãá?ÖhxHåW?¼›-ð†Ä?góoõð€[?i¸àaJ6÷?àŠì~T*
?ÃÛqY£N=?Þº@#—Åë?ÃלDÕÙ!?ï é|?«‰áô.ï	?èm?/Y£¤?Í_–âôÆ*?ʨåM2t?ÌÀH«¦Ÿ?w¿J?{]?¢Ðµ˜0k‹?éÝÂ
´§?¼ú?Á¼?ÇÊýtŠk~?¼¾Jqýæ?°ñúÑr?£9_è°Ê?ââw‰×ã4?¸ · ]?Ö"m›õü?·-Êu{úo?`
ÃكFu?^=ʝ;õX?â¼N±5d?¿(üðÎV1?ÚgåÛI[?¿>Þøsn¸PSR3FGL J1858.2-2215@+5}¡ŽÝÀ&»Ú@RÖgÀ9'Τ=aŠÀ;‹½÷FóÚ?ý…'MJ@C±Û"Ì?ð³!Ø?ËwúzQ¿ÂŽúPµò¿ç·f'¸¿í˖ìÁôPSRPSR?q®
¸=e;?vQ®?ï"¼†¿³p?¥"9N ä÷?—<ì{†²?¤xæ…Uv?¢í÷!±–ì?°Øœs²?åÜReÁâ?ÆãúÊи?Ñ靐Uß?Å@¨‹=Ð	?£ãô~ê@?'±WC+û?ë"å'Ñ++?¬`ŽYKU?¼öÙªo™…?¨‰¨Oˆâ?Ãœ¹Î\3?°ª¤ÍJ
O?è,m۔˜?¸4ùnÜÑ?¸yW­™‰\?¯Y'|ûº\?bÈÛÆxÁ{?pcõzñ?îóÏK	ò%?±b…ÐÞC?Ÿ,û)º51?± 1…«s?·æô7T=
?¸±qÞ?åMxd¦ÙÚ?Ãaï§Jåµ?ÎÖ¤Qƒ€S?À"²ÀÃ:c?²{ss?¡«"ÿš¡?éò±R?_^?¯	"(ùèG?½ïhûc…ƒ?¨˜òÜ=?Ó3œÙ®ÌK?²älB÷¶?ä~æàý¹Ý?´µ¿å¿ª?®t«'ÕiÑ?¢ßÙ¤3–ÿPSR3FGL J1858.4-2509@%ׄABÀoÀ)8!4x®À8Ý-?~À;7é;˜\ƒ?ðÓDá"@¸vb\ìj@Lú¿¤ED¿Ès˜•¯÷v¿èÇON6¿àYÖú¼ãå¿ï	Aš:eAGNbcu?ïÌLØ(~,?uÇ$4œM¬?q$–7z?pîï=bƒ?a®ÞuyÓM?^‹YBš?ìl®±·H?¹Ï‡7þZJ?£û}@Eàø?¦N‡™ŒÏ?²œÐ€)"Ê?´Ž÷'Ÿä²?éGǤfH¬?¯ëLú
›Û?Á÷:£XÎè?ªª
·i?±ÓM"ˆgÖ? æCéªLF?éÃò¯×Á?®œÚ›°ñ?«NÀ?f@}?Ÿõ´í(? 4#¯Bß?ªabûµ³û?ïÜXãñ×s?lž"™Í»ô?kGäg='ß?iŸa"RS@?P¾oXÔµ«?Hžøu¡?íýxPɜ?¬'³~?šG*"†½Ò?—9ÁFB?£å­nb´?¤$TÂ%ß ?ê¥Ý]l¡?«…½3?¿ùpnÒñ?¦¾÷Ös'3?¥¯IR[ ö?—#¹Áþ?í}ÿ•Œ0?"xkg%TÙ?¢ÁOMíŠ?‡zgºh?¥^·[рô?;¿+¡öAGN3FGL J1902.0-5107@u™ûoÀ6c
?ƒ£ŽÀ8}ík¨ÆÀ;{,Ü×ÜË?ýR=›¥@T˜"#@Ä Wì%¿Ð!°¡?w²¿äPàɪ·¿åÇh>Â*¿î9uýˆ+ˆPSRPSR?˜ùA)Rû?˜ë¿"¢Å?îò¥RÏ¥?žÆé嵜?d(û¢$d?vìá4KÙ?–ø—*ÿ]?°,B×휎?ꛂeS"?Â3ù¹ŒJž?²ã"@¹P?¿bz*Šån?½˜3ú¾	?¨qÒöË?é2ãìñQß?¯µÙ…ṕ?¸Ð¬؃? Žù,§'ø?²V±\ÙÊ·?£%þAcøx?ë‹\ó~›?­âR³¾7?µdóº@eó?¦ Šý'P?£¿lu ËO?¬AÕs¡?îg +ó½–?°QÜÁŒ}?‡C)Ñ9?‹¹l&å?¢ŠëÑ(?¬Â‡eĽÐ?ê°qKêº?Ân–Øìb6?À›³ð\ôÎ?¼ÈEœŸæî?͜:ôÇâ?±FO1"þ?åÈs®šÔú?±áÂoíù?¶ƒì£Ë¯h?Ÿ"	•Ù?Ç葹ÑG†?¨ô£‹Wù?èRWè8&ý?«1 Fh†?«8:—Ì'?›êWËc®5PSR3FGL J1902.9-6745@t} FÇeÀ:
%@+i:À9~s£eË6À;¾ç!â¨×?à8u_ÜA@Ü¢­¿ke@ÄÛ Ú+¿ãzƒC8[^¿ë:Û}ó)¿å9ËP©nV¿âógŽ¸ÅAGNfsrq?ïû"šæ?EwäìOí?Α^G2?.þW}c?>ç‰ÆUº?D¹ÂS]è?ï{oIäÐz?ŒŸÔBÎ5÷?pz—«f?}_øY‰±_?ˆç$8"Ûæ?"KCœâN?îæ>à‡â?)<]€&?†=Ïüÿ…â?€tªLžW?˜;é¤Ä§?‰û!ÒkP?ï éÒõŽk?'1V$Rn?Ij´àb!þ?H–ã¶8*Ó?†.ßúAž2?¸''Æ­E?ïáã+Ö?	?­TOۙ?
ðóNÌ
?±¯:tŠ?m±s2¯,?­¶2ˆf·?ï×¾ÿô[K?p$
Ëχ¡?V0c<hП?RØÂb\^Ú?m(Ρª\z?jENë¬Ö?ï€0x²ˆ?3´l£Ò?xÆftñ?vûW(ú­Ø?ƒ®âù®[?v?Ҟ?ïïb6^"i?`HϚç`?8w·Q´?.ƒ´h® ?[¥5cÏ?^ˆ9ä—`AGN3FGL J1903.2+5541@U~¤?åÉ@4‡ŸŸm1À7ÿ®õKqÀ:Ë>³™õà?ôźߺeA@¡Æ¹¸H?÷_~«+½H¿ÙžRÌ£¿ÕŸ=X® ¿Ú´!!sÿ¿á\äÓºãÒAGNbll?ïdÆ8^_?˜ÖYÌ ÀÅ?d¶´¹°èL?pþL¥?Ðb_nñ?—öÐOë?í×o?ÓՀ?¸Èô"úÄ
?¡;Hs"ÕÃ?£1eç±?¡MÊâOI?²Å‹Éç?êïñ!•Ñä?¯¬S,?±p\­ï«¹?£â¦¤€8±?·Dêª?§Ž¬Ê†ž?äky¦'®÷?³,OÈ4ú˜?²íÙP­†O?¥®•ÕïÕ?Òm–^¯@}?²ŽþÂr"·?ï¬"ì-2?¨{öª n?b8ßü?wV¿÷ž©ñ?€|vúÜuN?¦EÓN:W?ï÷$þp?§åF|ôÅ?'E%µ'!?—Ë»ír?‹÷ñƒk·?Ÿ¡Eôü¢Æ?ëçû?¬ãûÃ~q)?®yÒZԃ?£É‰ðZû·?±·Ê>Œ‰?£<¨<¦Ÿ?é)VÚ–Â?¤*Éѹ©?´ë"pçr
?š÷̈"?ÀäÚà‹Ær?Ÿw¢ŠQ­AGN3FGL J1903.6-7052@tEõŸôýmÀ:'ë ÍjÀ9"=çÂÀ;¤®Zþ‰?å8æg—Wº@¤ý)+@‰mèþ‡¿çxû@Ÿú©¿Þ*Y©ÙF¿å50ûdS«¿í˜™ç2«PSRPSR?é"ðåRL ?Á'†ÓTŒ…?ȀF}Ä?ÀòCŸ'Æ?'ÿe÷×Ó?_Äñº?à"\gED¿?ÉwM<Qr—?Ñhô¦¶ô?Ä÷÷é<«?̤¥á?Á¦tá~`?æ¡q,,¨?²ûÈ[•5?ˉ'Rþ?°ö%*™Í?³áQû0ž•?›–ì`ÓäË?âã$Ê\'?¼C{'*ß?Ò?{!?ºÐÿêäî_?Ïôt†§?°ˆ¡ßK\?íP˜î}w?°óýíoôI?´]œ‡B|?°SQ}úkf?w> ñ$?tJǃʕß?è_,€'Š×?©CŒ-®?ÁçsV¹Ë?¹ÔFhÅk?¹7µQ»œ?²ÎˆMÔº¦?ê0RæÔ¬?©ïæjHAd?ÁÚÓöŒº?¦püI4î?¦»fIÀPX?"'˜¨Z[?ë:¹¥[L`?£ó ¢×˜É?·äCy
ž?}Dwžà?¬‹Þµ¡oÎ?™‰N¦^ׄAGN3FGL J1904.5+3627@PÕlÿݛQ@*˜Ý ·0À:HŒŠ½À;»©°h8?)z?¾´?@
*)Ö=8ñ@ÉXŸÿ9\¿ïÿó´ÿH?ïþIãñ#¿âޔ`}Kä¿ÛýëJDAGNbcu?ï×NasÀ?'"•§ˆL?KG}¸d2?Sø7n25þ?pïß°"º?€`Aö"é/?íg£xü§A?¹§®^'t¡?›ññGÌ	"?Ÿ‹™ðyy?«ŒÏÉ»Ò'?´Ceš‹\?î(Tƒ¡þ?•æmjŽ)©?" )'d²?}è,œ²ã?¥0ç±-À?"'¼¼Ç6¯?읞b?µŽ_]@t{?·x÷_3?´v'†êe? \	0ÏWv?†×Káï?ïÙl$bØ4?­^KÆ;?M‡©8]‹º?‡ ù6¥N?o1ñ!'bH?§v€÷͆¥?ï>¸ª€ò"?¨ÇÒ?ƒO•!¹Zù?£	.x#Ø?@L j?—."wÉe9?ï)½ê Œ?Š—€ìwؗ?崃ŒˆU?pab;K•?'âû!ài?ˆµ€0æ—?ï`§$œ—{?"ô ó­÷?‡\²ˆ}èc?{¿ÂÚyî?€y"RÃòã?|3Ç=¥×²AGN3FGL J1907.9+0602@DúÀ%¿ìÔT@(4À5ݜ©'žÀ9êXR§lÁ@.[ê¡õ@ÿI@eË·@$̦·9¿Û²oË·Es¿ãfCo°+¿å‰¥ì@ãþ¿ìëè%óôPSRPSR?@'<¸çYÞ?Es[.¬‹f?î²K@M×?²‡'ô`zï?¤XÜ%Š?²t•Ü©A`?NUE5á—P?‰AÄ2ä?ê°ê>ÞÉ5?¶7¹V'¬?ÅÀüŽ?¶]éeõ?œ~´©x?•Ê‹œ.^?è9ΞÅ8À?¶ÛÌô(Ë?˅­U'?µ~§R\ø?Y³÷j7ˆ?W/{ÓÀóÚ?ì?ö#0d?°9­Pf¼ü?½™Øˆ·>?°'`
à?J÷IÅãq?[õ•ë¨?î`q!ôœ?¹£Ä^?©¿ƒ?¹~ó\ûÐé?M1ïÚá!§?{äË,tä??꩘•Á%'?°'ºµò5?Å<kº§õí?°&u²Â?£W3Þä?›­ïÊ¥@œ?è$¬!±€–?³ÂvìÆ?ʗ'é¾d?±…ë¹ÐZq?b©¶|9E¡?Z%¯wáh?ìd€\©¸?©(vu5à?¼F¯fà^Ð?¨ùƒì·pPSR3FGL J1908.8-0130@@ÇûÆnåÀ9±êFÀ9ªð]ˍ2À;²g†÷Öf?øçj@
ÌiûqOù¿ëyÖ1iH]¿ïqªôy¨Ò?íåO[¿æöË,¨nb¿í™\ZHö¿AGNbcu?u‰Îô8i?£"×}w?îãî§a?±7t>û?ž<n~	†—?¨~PU?}ù̇r§?ª¯8L®¡—?éy+_ Ä=?Ê491hǃ?É+"+`Î?É~ùù\Î?»ÿFO‰o?¦ÚÆM–[®?çßkIhîp?²—Š¸L¯}?'з4‰?«ð\ø=8Ò?³¦ÏgOÓ$?½m"h·?ë¨ü&íC?ÄØ$ j¼?®"Ÿê¦‡?¶ËhñÉ?w"ÜÓ¸?•z*U£|p?îÜ|ÛÑU%?³iy{s?ž‹¢—xC?°°½9½?…JŽpP?£/îò¡:?鳓á¬O?ÄVÈ¡økj?ÇÝ×óz?ÃEEj©}N?ǖ°TµÓ¦?°A~£®w?æQ´ÜÖ?´×ß^îÐ?À$Ùÿv~?©ߝšN?ÀÜS¢b ?»D}?hB+?é–LaqMå?ÂéÚØ0á¨?±"õ°Ø?·¾3PSR3FGL J1910.7-6000@u"§e4À9žÚà‹ÆrÀ9ÚïÅYbÀ;Æ{…²\?ô£D",î@ÄáÖõÈ@š½ …«¿ä»Û®ã¿Ù·°ÛÕ~L¿çæ"gÞá¿í»ûÄ1OTHERglc?¸à–2{?³æÛMØ¡?ìb+™¿aÞ?¶'Ëá··ß?"N…GrÈY?"ÏK'4x-?ÕT'ñô=?ŕÕ1þ³W?Ý^>.ŽÞ«?È)Ë,±h?ʛ\~þZ0?Ářz˜€?ØĄH''?·³ÔêÑ»6?àA¬®Që
?¸Ý`ðeI?ºà‰m&žû?¡mf¨ßx?Öm-f%à?´%	ý>`Œ?á¶SsÅt"?¶p㜏F?º/¯§ð@è?¦º}¿ÉY?ÁíË;?¾úièüÙ/?êÛÂu¨E%?¿ûƎ³ü5?‡WCº"/	?ƒÎÄ,ïê
?åD®Uñק?´ÖcùÎ?ÌüçŒõ­?¿¹ÔïÓY{?»à¿!WWo?³m²·­?äÀOp«Žº?²|*ô–?Ҿ䪗¡O?±š´'J­ß?®ã¡eðê?•€R@´Ò?äÇöéxKŽ?«-S
Ä4?Ó´g°éAx?¨N‡Œ×?¥ÝSâ
"i?'ÿðOX¹ÈMIXED3FGL J1910.8+2855@N{À?ö@!ƵÜê&À:8ðvö£À;€d%C†h?é{noc)	@
~†ܖ?÷jŸÁ%ú¿çZÝ÷lˆ"?ïÿª,cä¿Ùd¸&'B¿²¸oÕrZ2AGNbcu?ï¤ÿ¡¾ß­?Šô#i@Õ@?Tz‹ðbJò?SГ•|Â?"0Æ]g?‰î1Ö?îV£ì‰ÿ?³d´éö&?…ý°Å¦?Œ¥$̙õU?¥U6P9¢?±‰ºÜè×?íkv"cÏ?¢Žçb?"éŠ
X¯Ï?ˆ'T¾¹²À?®ÓÙÓ½Ï%? Ã þ7´ê?íŠÕL‰V½?ª¤ó0b3?¡Å{s£L?¤©Ë3"Iß?¥/Æõ¥è?¢'¹†Œ8?ï±ÓìÉ
ó?1ÈC?B§Lͯ ª?Aã»X:nc?'`óŒ®ì?Žª©(±8Â?ïd_¢`¾?™Õú» ¼?s]y\D?yZf©†dq?9°ì?°y?"±Ô[3?îYãg)@&?œÜÐGx?Œ
UF6#?ˆ "à)ËÖ?£_&4ªÔ?˜ûbLÖfa?ï'@iI?ŠžòÛ–Ý?Ÿâ¹;ä?…%Ê;ŽP¯?†ŸÍ%½G×?}^ÇÍ:ÜAGN3FGL J1910.9+0906@E ßÔŽ¿ÃäH~ôÒ¥À6k3æÉÎÀ9–M$v?ú´'ÇÅ&@¡NÇѐ?ÿk"Æ(˜Ð¿ßc%  ¿ä\áýál¿àUf.2Br¿æ´7À
DŽOTHERsnr?[:î7ª‹?VóŸLÌñ?šOdÏßè
?¢*r»Ñ€O?ïçÊæ(û?¢–êþì#?_6aõ³?ró²Iô?×(ÍWûÙD?ÃP:±›ˆ?ä[þQáN?Ã[_þ~†Õ?²þ¶ud´t? éFB>ê?¿CwÔ´?¨AãPý•?é·ÈB=V?®É¬Û
•??–´ú@Ä?"$ϺÙS?ÅTº;–$?³CTPÃ[?éõ0¹äÆF?µs5?/ž\?d8l
Ív?s¯~ߌI?¡¼®2-)?°@+<!vü?îÏü°ÑTØ?°ñà1*0?m¥Ww?€žVarv?àSme^)?¿DŸJ´?ߌveb?¿˜òY.Å?½ÖIQœn¥?¥iJZ6ð<?ÁÖ¸
â¡?¨¤ÛY<
K?çϖèS)â?°XÝæË\§?˜N5zÝ­?š–Ðïï?ÍVr™`Ê×?±Æ(R`sS?ççñ­ú1?¶'¢â¤—¨MIXED3FGL J1911.2-2006@0â
_ÕR­À*sç_JHÀ7ºÚ4"\À;Êʔ
i?óusºaæ$@´›Ü¿ß@E¸7~¿ä_Œ+Hk¿å¯rÎ"`¿æԃâu¿ê]8ÉÛxAGNfsrq?ïߕ¨âü~?kÖwMh?Uö9n¿Ýò?W9mÁBå·?eo:9¨"k?gý¢8–?ïl×dËK?'i®,i8ª?q±cìÄq?Rì¹½H?‹ñ‰Ê¸ƒ;?Š(JdÊ?ìþW2Z´ñ?£ùÏÙ"?§°Go19?˜ÑEóÎE'?¨jxQʸ?š2è4²9N?¤ëdñ?ˆ	,ËüGƒ?L™VÊøµ?Z^ —H?‡'}>ÆĈ?‡Õ›*ýÕd?ïñéÆúó?S½©Êcmè?J·×Cñ•?HPûñÏÈ?M¡
rü¼j?F✽yF=?ïʎSÀF'?x¦ÚËÄ3?\³(w÷•?Y¬~CÂ?sŒ>±ë?s"æi¯?îzVÚq?˜ºv›Ù3?š'µ‡?ªU\0‹?–²'rýñ?Sºn#¿»?ïëZ'O
?b´ØÛ=à?9ÖpKá©?6¤8°¤R?ak=•¸?aáï#ðmAGN3FGL J1911.4-1908@1ÑŸ>õÀ)½ôafLeÀ9j+Q½aöÀ;6dE#ö?£7.aߐk@"î´þúÇ?üQ¦áUÅÚ?ïµF2`Ǹ¿Úá–|y<¿ÒèÛµ ®¿ÖŠÛÞ$AGNbcu?ïòì–82™?SWÃóα??ûcËf?9öö}à?R'ú³K"«?N
ÿ_ê?ïè"ÿV?©})aÓM¨?{geù?'j'Ñ2‡?˜A\I?¦†µ"õm?îe:Á¿Iú?–Æ®³»°?»ÚD?~ÛŒPðX?¡èQ´8èe?"Å÷a!D?ëñ¤¤~hÕ?¦7Gû"gâ?po:1Áyv?oºyF;›[?¿kç7dο?¥ïÜÞr#¤?ïù‹Œæƒ?G`o¥ov+?34ú¶Î?-'|û`?BTöc}?D-%'•w?ï¢>È?ŽÁœBy9?f"ËÙN½?eø>ª/Ÿó?êߐ–\?Š6`	6'?ïUS—_`@?'{­Îlx'?€ì:I~®o?n3&Ït?‰¾ßÒ¢Ÿ‰?€g'0§¼??î»îÿkt?ˆ!÷0•R?e23L?Rà.bª¡?¢ýðk±?ˆªÓß­ÓAGN3FGL J1912.0-0804@<	I`œ"
À }ÖOÀ9~ø&²òÀ;Œ#QA¿É¬v|DZ@Z¼#jR@\"Ý¿ëÂÏÏÐQ+¿ÔÎ)¦cú¿ßrצQ'¿éú–«õßAGNbcu?ï£×jW>?‹C"V¯E?­]5°$?‰#²øëWµ?es!ÔØÝ?c"ÒG›'?íó"N%I]?°CIt]âï?†'ÕZZ¬ƒ?‰0fï-}?«=ÅÅ\ñ?¬v,Ȅ?ìý³9ä'?¥u8ÊǙ?«¥¦FŒJ?Ÿüñhôœ[?¤(m÷??"Úk›Úf"?ímºÌ«P?¢c™œƒ8?sQ"MX¤?lÿ!ɬnw?³]t3Ì?¡É'wæD?ïËz†€?{‡ü0»%Z?ujêÞÚ?yiƒ@Û?UKy›
?RëvSîèt?ïG³o‡9?˜Žu-'y?s¸"§
?tvd&@?'Ddñ€#?"á&`'™?<rՓ?—3b,?™³¥W"›Á?"6ø¢"?¯&7ÿ±?…æñíìÎ?ï©Êòµ?"ø†e¿Š`?c/Ãxûhe?QÇ^|KÐÅ?š"Î7YSF?ƒôvRK`(AGN3FGL J1912.6-1223@8+OP À$‰®ÁIÀ8Ú7æ÷~À;!•ÄøÿÓë!Ùf¹@¹ø`Nt@ïÜÀŠÊ¿çƒÌZáøÙ¿æÃqù[dï¿ä8,ŸÎÅ¿âñn±}UAGNbcu?ïñk÷?WÌ''pH@?+1à¿Ât?(1Qѳ3?YtIµ»?VeºÉƒ,?/Ác¸?ª,ÉÃã"?h(Q
©Ù?†>{Êè^?£Bï\‰?¦å||?{?î¬}`lÁ
?'-t£2'?ÃbAí?B4ÀÂv‰?›Ž¢ÕƒÓ?ˆ­Bàþ?îzwòt?'ì¿`œ†?["¢}"?U£ºàÒ?­€;ê/ìÔ?Á÷NÙì?ïúç°äõõ??ÑJU•x?$™w"¶E9?"ÁÕÚJÜ?>u½8Ö¾'?:*ZÙ1•D?ïhy5ËéÎ?—VBp¬ª1?mÅÓôˆLp?mS(¥÷Z?Žp=~"?"]ñ¢Åm?ï'nZK?yŽ[¢ƒ?yµ Ö7ÑF?qêdžG?'‰¨Ž•¶¶?mIÃUM?ïû_©«,?rð»Vê/Ò?FV¶–ͯ?5op8+>Ý?Ž›¼¾Êœ?r³NP¹äAGN3FGL J1912.9-8008@s <€"ÞÀ;c¿ÂùÀ8²gˆ¥UÀ;CE?¥1}?÷õýR{¢ä@ÿÿL%óZ@il(¶X¿àøm"—ø¿âøëÒݙ4¿æ€;WM¿êŸ½¨ %AGNfsrq?ïÏ=REòþ?r®Œ?páòVš?m£@`g#É?`"ëÃ¥4A?^ƒy&uø?ïb‰+ڛº?'mÓÄÂû?rZ­Ô˧?~íEXÙ·?Ž0^-¥?Cþ‰k ?ìlI¹KT?¦FM—7"—?²M'£îìŽ?¢·¡Ç"q;?¤ AýBÙ?"ˆåèØë?ï;¨˜m¨-?"`†õÊih?nî1ɓ?ráê	®]?"­+†fm?"QÁ»7(T?ïíÍ}CD?Vx؅ôë_?X…ìr•Wð?R
I'œ|I?G¾1èïZ?@HåµÐ[}?ï®uô£Ö?wdçó˜v?`z	ÆOG¢?[þ~´/®Ú?vkÀ1¤¸ë?s31Ú:m?î~^!ÉSq?˜äÛºº÷?Ÿc<R{(é?"‹u¿tʂ?ÐÿyÒý?…lSö,?ïÊÑ͒šw?rò?d!-¢Ô™ˆ?[•´ø¼µ?p†'nç_¼?n»æJ%)AGN3FGL J1913.0+0910@EÇwàmò¿â:þ Œ=À7éç3ö¨À9ʜcxu]?ý"T¦uu"@
Eq•n'®?ýiš¨¸E?ïÿf#dLõ¿àñfœí1¿éíM¦¯ŠO¿înÂÛ(ÒPSRPSRP?*Õ+|˜Êl?/df".±?ã¨M©ñV?ÑÂ7Iº«"?ج9w£ƒ?ÑÂ?$Øý]?2_»"g Y?GèøFW[^?ãrŽß¯?ÃyˆNý[?ÙJSO!??Ã}â®áTn?Ší±9lŠ?}· Kœ?⮦j×Ã?½'«€ ÷œ?ÙÎ4Uòû¶?¼ô\'	?t²ˆ¿0öÑ?sR…‡ã"ˆ?à-DUGZ?ÄDÛW»9
?ßR­¶Jï?ÄMæí=[?]Zp+?:¥øj?ß`
Éc®?ÓQ˜iÿß/?àO‡¥ƒæ2?ÓQÚ¤"b?I+¼$µ³?d…ß"+ñÍ?åCkH3±™?½
­˜Z?Õl"âšO?½.µj/Ÿ?•Ütcð?4´[9?âø±ÙºÏ?¸åÙd$?ؽކÍRó?¸›^žŽ$?y9¥é*ö?y»´ˆ´?ܺo'nÚ©?ºdDÒ©?ápV‡¿?ºàY~mæ…MIXED3FGL J1913.5-3631?óA« §UÀ3å*?nªÙÀ9·ä$gÀ;qBÖ>f?؟ºoýéÐ@lôÂ4B}@K^ tT;¿ØÎÖ1¥i‡¿åNGÉö·5¿ãaà·);Q¿ãÜQFAGNbcu?ïýȸÇ?,w£Mñk?͘cw!:?Š8ç†â?4PPÖÕ{?)™ãÍ?ïƒ55¨?ˆ#ø™™?l¦G¤ř?n|L£
?ˆ Ò?"?Kqyß$?ï9†¿ªØå?±ü»¹?ƒ™{ô8'Á?söTÏrëñ?ŽÔáè?w÷qdfôæ?ïɲ;¯Œ(?u¬ûð'¥?"ð÷*Ö>^?%ê¶(Ì8?zZ€FÝ?urî‰È…?ïÖC]ö?¯6n9å)?tOP.pr°?¯7ÃM[Î?!å0ð%Î.?Qvɏë?ïՆ©Ê5»?q'Íœlù?V¨FéEà?UJ	‹F?o%2–Œ"1?kÁu,/9{?ï¦G¥R'?t£÷˜Ä*?sÿ¼‡{?n¡•­cÁ?xÿ¿ƒ-/…?gmCí ¯?ïõ,˜Ëy¢?Q¦¶(î¦.?³í:à?`œ1Ü?Tò¶—´?Q*ãíFˆ.AGN3FGL J1913.9+4441@Rö+`Ø@-÷™ÿðæˆÀ9úâénÄÀ;ª
ájÃ?Ü<<
Lo@F¯ÀÍe#?ýužèó¿å07õËÛ¿ÔúòàæN¿ÔÔߜC~@¿Óž£:†§AGNbcu?ïnk¾:Û?¬CòH1r?X¶É¸í³&?_ò‡?¦"e?§11Ñ3d?¬.åD®Ú?îpcžú›V?²F?côðM?¦L¢ždª?'±œØƒÞH?¡2ëú4p?­7ʵ¤]?4'âN?ŽÛnÛgà³?ŒbyXÅH?zÆÕS	|?ž»ü¨¯!›?ˆ›™ØM?íæÄIŠ?¢¶÷§°¢d?""#†ææ3?"j‹¿/c?²XFþl,#?ŸÌùì‹F)?ï9h1uK?º€UÇvæ?MRòž¨â?k™D‹Õs«?—æ@¥6±?º:'ö5ž?ï ¹§';è?Žw}…©Ý?oàkÈŽ"?lã=I["?²ö8PÚ?‰*@"û3?ïaTSi^"?{ROþ?²]•©?pµ¿•°Ä—?‡Ñã†#zk?ræäˆÒ¸N?ïòîä=œ?'Çn({™?‡æ½½&?wØ؄H?ŽC¡«»ú?y©‰é²½€AGN3FGL J1915.9+1112@FÙIàâi¿Ñ._ܒÀ7ý:8
2‰À:;i…Õ—w?üÐ=‡Êå@‡žT"Vå@6ßïiYá¿á­å_—¿æÄ
¡C²¿è>ÓåÅ¿ïþ—ëC°YOTHERspp?bУÊ¥6?aÍ´ƒÕ&?ÌJcë% ?ÆãP¦ÐS?èږaßK³?Æõ©9õš ?BÌi%"ÖV?Z>°qyÎN?ãõrÑad§?¼Ÿ!ÃÊ¿?Ø´(¼ß?¼¡Ó…Sç?µ¸œo–=?£ǗŠžö?ۚܪaâ?¸áªT)?ÞöüNx;¯?º™èsò@?"L}ýžá?…úž=لŠ?âîµ­vpJ?¸q<¤çz?ØòÝȟ?¹=øVdüß?_¨Ü¾Ã…â?f'Ú(í—m?õ¸˜&A?Â"Zbž
?ëH®#á¨ô?Â?®ZŠ©Ö?^§~@*m?sœŸn«ëg?åmªÛéÔ?´ã'Z;ýà?ÕÐ},6ÐÞ?µ«òŸŠÃ?Ã;öndj@?©ƒáÕ
?ÛYMÖä?¶;Áá²3?Ûð{Êóü?µy±eËÞQ?™´Êa2€ù?g¥NÛ9µ?äIÀî, ?®;@¼Ácx?ÕÑ1|`	?°‡e¶'l¼MIXED3FGL J1917.7-1921@2<‡`±ñÀ,§Úáb†À8'Yáó¥À:Îÿ€¾?ãÊåÁæ?@'"T±I?ýòÓÿñè:¿É¨còÿ͑¿ÜøÉkI¥¿ÝF*ú¿ÚÙ©Ê>R AGNbll?ïËÑgï±?qF"õR…?N ð¶¢Ïç?MeµÖoæ?vC-ÜǼ?n˜N00¿¦?îŠo~¬È?²çE =¹?…';VaCc?ŽŸW´÷âÞ?¡ô¹B.ã=?°ažp7r?ì*Çð!Ä)?©ÕŠqĤ›?š™&àÚ?c!"ê…?¸vÇ8Œ"?¦•GçÏ?èK‹.?ªŠSj0+‰?‰v¾õhÁ?ƒ=@Ò]þ?Í:h!—³?ª=8 ¬°?ïè!àá'é?aU£^‹?Eù¾åª?IæH¬ý@C?bšàŠÔÁ?ZÄŠ
vL?ïiT4Š¡.?žÓ‰¨«ro?s•.±V?yrÓ;Ž¼ë?‹àf=¾ÕÓ?™FQÏÔ´»?î‰~ýÈ(‰?™¤î–³ü•?Œ0Ï÷;Å°?…¯ÜÉfˆ? [Ü">ê?•§ëì͞.?ìÆ"ŽdT?"¦'?"Gk*n´+?o·ÝÂâi÷?·F]ôE`?"Ÿ
ªrAGN3FGL J1918.0+3750@Qqb¿è¸¼@&äÔßÀÅXÀ:jå€!ùOÀ;ÅÃqÚ7ï¿ûŠ­ Œ§ï@j£¼2K@‰_²?¿å_Á¤$·ð¿ãÞOªüÝ%¿Ø¡=6÷ì¿ã«ìE@¯{AGNbcu?ïµð½Aê[?'1SõI'v?D}n¬ïD?D¯h[ÖÝ?;ùÁO¨£?¹áú7¿a?íø.Øäè?·d)	v'Ñ?',b3¦Ë†?!¤¶ë7?«ñùà‰Ë¤?µÀº«†,à?íß¿wñöt?—µèVV~?'®"qÆB?hz0&r2?¨¬ÆGýŽ™?"Ïy
Ù?ï*—z§ÞM?Œ‡Ø¬¨??°åáÍw?A+Rn>?š.M2"?ŒC/™d"S?ïáû®v?u&Nì÷¸|?;FDbž¾'?EquþÊô?jœÜÙÐ?s½ù˜k!?ï˜ïpnZ¯?'ï+‹7ðÌ?f¾á0ã¤?l¥ßmÑNC?"k}W?We¬Lè?ï*«?3qœ?†Àð?"'°'ð½?}kŽnOÿ?jÎÈ(	?~VSµeþ9?ïÕ#è‰ä?e/g]DœB? h'ï]‡?†W¼¨¡h?têÇ?·S}?dñòXAGN3FGL J1918.2-4110@vL» 1ίÀ6=QÀ¼ôÀ8ŽÄ¾áQ¿À;E%£þw?ù®:m$¡@Àn&nª?òÕ5 É#J¿à;Y2~àä¿Èì0g"/¿ÙÖwø×d"¿äü/Ö(ãpAGNbll?æ±Þa<Ð?ÈÆ){¾V?®¨¡«S-ä?±ÿÿ@qÈ
?͎^®(G?Æ¿ùÙ?æ¹aÿ?ǚ¿Z.°Ô?à ÿ‹Þ<ƒ?À6/Á'–â?Áú¾ïáÇ'?¼;&q®Ãø?àœÝIwî?µöªÕä?Îÿåœ5¢?³‡3ía‡?Ό¦Õê¥?³ôˆá7(e?à®L®{ËJ?ºƒÈ·?ÅnçDÙ_?µ$¡ÍâÐ?Óëó›¹ã?º#×F^šP?ê{šÍm©?ÆÐöxÓâ|?©ô·™èR?²7/ûœù2?ÁE
çö°?º>%Äo?ê²>ø>Ú?ÀRBœK"m?·/Õð1ã?´WÔóÏÕ?³Xߛ—±É?²—«fåV?âq¯«\mG?·1Ãr`8³?϶3Ê"È?²Ø²n+?ƃ
†Pf ?°"ì98U¾?ä4jrϚ?°gÃ"ÇW?ÌNŸ—¬Ò?ª\ÚGDô7?Ã#	FÆ?¦õz[SAGN3FGL J1921.2+0136@B㭟àÛxÀ‰¦ ¿çÀ8Ý^ʐ²À:û( °z?à÷èόš@…#Ôñ^}@º 3§!¿çg.ÀæBG¿Ø¿›¾Ycì¿ä`U£ª?¿í!5ÜI±>PSRpsr?¾ÒÝník?º`.~m™6?äþÁTÚ³ü?Éq¨" r€?̛‹ìݹY?Æ1
"?¶ÿæ01\U?ºV""Õ˜+?ÛύB.‰ç?Ä1Jr6uª?Þpy1;®¤?Å]"þhêê?×{‡OÀÁ?¸#)êæçv?ÐÛ"õs›?±ëeR÷?שVªJ…¤?¾$p¸#óO?ÏLSã¾?±³Htìn±?×­B–±‹?¼•/€åÝY?ج|Àoò+?ºkèÏji‰?Æô&¼ñý"?Á~c6Ÿé?â¾›!^?Ê=­¾cl?ÎÎدrä?ÅvêsŒû¸?Ñà
l>~?É!úÉÝ?×l*[ÚW‹?¿îRƒ…†?ֳˌ¹i÷?ÃYGój#?ãÚ§3"?´ô—……?Ê`ós2ZN?ª²˜\|$?É Õ"0×c?±ÄÏyæ¦?Þªe.X ?³oµ¨??Î2N<û?°Ïû\œ?Ò<s‰öŸ•?¯IûÕ+žMIXED3FGL J1921.2-1232@8ô¢€Èè<À(u¡ueÀ98äŒÜòµÀ;A_~Ù?ᓧº[(@b~Ù$@Ihßg"?ìíbM@êE¿á-V>>ï¿â2Çc½{¿ßڈíÇCAGNbll?îöÏm:I?œ
²< Î?'bÑ?~%-=PD?—õ§Dwà?˜'¢÷ˆ¯‰?è' m/?Й6]ñ3?¸4QæOö?ÀÄÒ¾ƒ|?Ão÷˜Â
?Æ­oºM?ì$Ʌfÿ?¢tÞ6ž?¥….uÿÏ?Žå¾÷-?´|Uœ™È ? 3!nÔbÝ?ۃ'Õå'Ú?»yx€´?ÂáÑ|ðý•?¶{U«(j?Ûïl´ß?¼ÞÖ'A?ïe¶MYz?Ž(»*Ñ?z!žFåµ,?‹M­fI?‰|ç­?"ÚÅmcÙå?ëiy_3¶?ÌPeß¿?®HÝ\š"G?ºœsØXµè?µÆTÍ1®?Áf;y¹æ|?îj¼<dgç?"%-ŠG"3?"šŽŒ]"?ƒ|ºfqç·?Ÿ
éì{?u˜VÀC?æÍ¡'³Ñ?¯™ï5¡Ä?¶ÜIœË? Ýó@ˆ?É[U0‰	Ô?­¨H	—AGN3FGL J1921.9-1607@5´ß¿ØÀ+Èô^â
§À8ý»V'ÄÀ:òéû±¼¦?仍_Ø
v@V;mê>M?ùØÏY§f?欄ñì†?ËA~ÂRË¿Ø	žBI¿ÏjØïx{ðAGNbll?ïs<x+_Õ?¼jæVø?d:o´61¤?c­.C®¯A?Ž"FœN?²ˆRõEg?î¡ùu³q˜?²·dÄû?†š8Ž_?Ç­Ë¥? YÂ\Ðã?¯¬­:¾Ë`?뺱}w5R?«báâ…1?¡^Â÷¥Ø?"àŠ[óx?¹{—à›‡?¨QEþù?é8å3ö҅?´ç>+?•™#ŠÆ-|?'°ÿ•5¬–?ÈiFÀƒ¾;?´ó´•üߘ?ï°)Þ ´Á?í‹ÍíÍè?S C¤güZ?RQ¥«ŸýH?'ß&HA?ŒÕµ#—m?ïu¶ëÓ½?žÿÀ²:¹à?ri•uêØ?}+ï©7ž?‰‡‡z0"^?™!pـ;?î j%¸¡G?œŒ7Ü:S
?'5¹®§É?‡ñæ
w$?¤Þ€Íq—°?˜ÖAWț?íñ§ýa?ž`Вc¡?‰€,í<£?x/8¦?³øm)°ç?"¤tÝÛ:AGN3FGL J1923.2+1408e@HŽá@!X?¿ÝŽ™¿óå.À5É'm,SÀ9'Óˆ¨°Ž?ÿdF0eùY@ñÔÌËu4?þ«äÐ(Í¿Ø3)˜—¿âÏ^w"›Ü¿âÐ¥Õ>í¿ä®ÀýᗵOTHERSNR?u\I-¦ß?v¾µKÏS?¥ïkç'rt?±bETÅ?îvP¯£yË?²+VG+Úò?Y·çëê§Ý?pqÍϸ"?ÙE]·ì?Åsƒ
ó	^?ãPu0X¸S?Ňaú'"ì?±%½PÜP?¢ÚÒ:s9 ?¿qR›¶ÝÖ?©>'—.Ì?éí–Õ'?°™Gäp-?"n,©7c?L¶3z£?ΘW š??·ùS䧶?ç¾xҊã?¸™Ç:Ÿ_Ã?SŸy¬c&?˜ÃNZT¢?©uâ¼Ìo?²úzûÔ	?î#`Dß?µó¾ò?hTŒNrd?{²=àLd¿?áp;>W²?ˆ8ñ쟄?Üîà®-ø?ÂÂác]È?·Ûnšû4?£ÿœ&rÎ?ōܳ/ÿ?¯š¤µêN?ç¾îµªÇ>?³<y8S˜?—×ü` A¸?"g,eâӌ?ÒÁ"`…âê?¶B˜O†iÖ?åàuì@ZŽ?¹¦H,(MMIXED3FGL J1923.5-2104@1.¸À¦MÝÀ0A'ÿùJÀ7û:Þ"_¦À;1!àûX?ýÎrn²eB@EÍNY?þ6¾¾P¤¿Ø'#_3¿áñ"þÏÿ1¿äay¯XŒ¿ìÒÖ{™ ÈAGNfsrq?ífÛW	ã?°ûÖ'‡?³žµc–Ö°?¯÷¹ffÜñ?r§©{ÿH?p8øæ¤mí?ïvgÓ"Š?Iy+\?pJ`Ý9q?tó.êÝÜ¥?Š@ëðøû?ˆóaÃÒ?â€vQ¸Pá?³DÚ4b"?ÓA&S¯].?±UÔßöI?¾÷´'ˇ9?¨¢"A<í?ïÐΣܜ?€2c22	ñ?CÌØ#"T©?cvø¼‹'c?u£ë?~ ž¦¶È?ížço±­?´mômXP­?±¤¦œÝ&ÿ?´Ïcm??vBô%mV?tôh;Å×?ïË¡ü6Z?yƒÌý˜øW?^Rœí"Ž?`ßÕ8dI#?ršZ‡Q—É?rU)õOŒ?ášGc'?³=ÁD2©?Õ݄^êò?±+W|h±D?»¹UCÜ·?¥).}úi?ïö ´DZ?WËÅ ×?7ßsݸì?<µá"×?KãĬ:åp?T…&Bs?AGN3FGL J1924.8-2914@"´ö€$}ŽÀ3œ`ÔV.À8+¨¶mÀ;@)8Þmß?Ó÷#óC@0ƒ¼7©:@F¿×ñÄ¿äVÇâØ'¿æ^òŖû¿ç¶1<¸íó¿å-«eã£mAGNfsrq?ïìð¿×W&?è%îÿ(?4Ù¤5qü"?RÕüÿv?`tc)™?}uKy*¯E?ïowó'Å{?"h@%÷ðÄ?pʎåþ¥w?}DÐ%/,?‹¼»´Uðh?èZՋ"¹?î`õª«Sš?—31ÿ®*Þ?‰Õ$˜~¶?}0›2³Ìð?£{\SÔB¬?•ÓŒC?¦Ñ?ïn‹b–›?bÉ
æÜð?JJHƒÈB÷?O>Ñ7w¿?'mœKá¼?Èlæ";?ï[MôT¦ ?¼Q~ø®}?SÊùÿYË?¿Ê —£—?"Y'ÖQ'à?»(""µë?ïË0¼µÏ?t'ª·èg?[Þçc÷U?VX}æ?s£*Aë}?qd$¨|?ï5òœë?ˆúïp&P?p¹.ìóÐ?xv<z—'?'eŽ£gé?†5_Š"ë?ïàŒ.÷‰?k"á^ʬ?01&ýÐ{?'YT øæq?mm¬äv¢ú?jÑË~¶ñÇAGN3FGL J1924.9+2817@N篟•\@kDß­úûÀ:p3SêÀ;~ۋ¬q
¿ãP¸t{'@DÖ(–!?þ$º_ÿ¿ïÿûZÔ·Ó?ïÿ'IÏ_'¿Ý©ªFB¸¿Öt¶©R|ØAGNbcu?ïð'þéj?[ ôaOG?<Õ`z0?6ëv(€?WÄ«÷[Q?XÒlÁðµë?î(}Á2 ?°×.Äg£?€qWî?ïr?"ÿðë®òï?©[Íô#¯±?®ç	¡ÚÔÏ?îMÈö(Ã?–¤¾œÐ‰?ŠÃƒÑDüj?x²Õ<Î`¢?¤r¦'ÿ»?"íDiûí?ïw
QMá›?‹âÄo€øU?o"gÄ ?|P7­mÅV?Šx†¡Í
?‡X"¤µ™?ïú§År]??ì$ÌpÝ?%J5FPS­?64ò²Ô?@:àwh?;†Î?AK?ïx(R&	÷?•¬¦dùÁÝ?e–§éì×Õ?dv	8?ŒAnCÜL?"ÕÒׯ.?ïJ±~Š?…á=r&c?{¯¢Ë–žÂ?hç
¤í_g?{Ï]Øx?"	m"^–?ïÞ,~
L?eöðöAw.?DÒª"<?:TGñkÜ?lž×]Ñ?e5x®¤°AGN3FGL J1925.7+1228@Gõ¥À‰d¿üw'áC§JÀ8'rϏÀ:lêÔЦ?à¨I¾B£ò@ëºùe²@Øó_ތé¿×W}ê*o"¿éÊhó‹Ë¿çF:*.î¿é.ð^ÞmðAGNbcu	?è#Qµ§ú?ĖÓmÈ&í?Ÿ'NäRJ?¢ý¢Š\yx?ˍÏi'ÉN?Ö=.3Äþ?×ÈoU"qD?ÓQØB?´.ËÌE?®µ>vï[Ô?á™â|ý-?Òa)H¬IÓ?ÚzðÝ´aØ?¸Ÿ"ÒÅÍ?Äi,M?¬í'&³¾¡?ÛzښHsÀ?¸Ã1öi¡?á6Ë°ºië?¿ކ;KŽ?– þXҋ?‰VúÅI?Ü(X½ö	 ?¾É׆Üu?ëvœ«2ñ?ÂÌŠEÇ=?—عçƒ6 ?Ÿ—:r+fl?¾Tì/WuL?ÁrШN"?âúÕOÓ?Ô2¯%ƒ-ƒ?­ÍcÈ×7?¤"¡(ö?Ø>^då1ó?ÒWû)+h?ãjV½üÐK?ºÛp$fwê?»éٕvä?¦O/Ô^/™?Ò1
¡²?·!ͦ@ºé?æÇã‹wP?³Ž¹'ŸÂ?•H>+Ýl?~ˆ°±lØÉ?ѵ‰6J?²òFϵvMIXED3FGL J1926.8+6154@WS*`%څ@3½¬ÿ§ëlÀ8ªlÞPÀ;6w†IZ½?ñB%)[.@Ó;.ª7w?ýÓÁ`]ö¿Õ2¬inÈN¿Û;¿¦@Œ¿Ü4…²uÍ¿Ô¥R?=¾AGNbll?ïø3o
ª?HXðÉC
?=Wkˆ'æ/?9è	ÌëÏ?@†wÒõ8?<êG	—?ïn¨ßT0P?˜¯­úq<?{
аœ‰?wi'z÷Y?†Îßßi«—?•Pð¯ìF"?î}ùŒë­°?˜Ý—ƒˆ?•r£¸5Îß?Œ_$4Ú
?šÎ*¯{å?'¸½Aµ¹?퉊#@20?¡QÀ\¿;?ˆÑå¾ÊÑV?‰<Aré?°™r0JÕÏ?ŸJkÔX$?ïýxJ±?,¤ª[,–?'EAíÝ?",SxvÏ-?!9ÆKŽ[›?¦û{d¼?ïÆMjµU?‰†ŸiƒÒ?eŸë¡Ýã†?`º<e¯±Ý?r	U+ex?|ôè™äDž?ïJR»}ˆÜ?†ûY"??ˆ»|4²Më?€tĎãO?"¯Ôè{ß1?zLq1r÷?ï9nÁSÇÓ?'jR¥…ˆ?ôі:µ?oÿ4?+×?F-f«G?öž4
'AGN3FGL J1927.7+6118@W0€5D…@3mù³>†À9'&µvoÀ;€‡6À†m¿óؑÇ=@Ó@ÑÌf rý@#oÀbV¿ä=¾bb¿ä
ËHp夿åQ ¤®SC¿àÏ	ñy0AGNbll?ïîfŽeš?Sžê"hœ[?I"ÕÕòm8?DuÈã5?Vhxna–£?N·*zI?ï—ÖS'Ö	?ó¥UnÚD?pǶµû¤M?oZZ†Yý?¦ÊÛq?Œ_øIc‡u?ï"ƒ^Þv‡?ˆ»ˆknÄ÷?†ììf•í/?{q%°y1?9ôUÔ}?€µ¬´þHÌ?ï7›}§ÿ?‹›¢¾žƒ?JVÁ±?Qd¢[%è?˜8%'4H?‹GǺ B?ïø¢
äø›?Ah&³'zä?<4¹ñ"º?2Ýßߟ?>ºØ@ w?9Œ(¨)®õ?ïÜÇ— )?p¾³
A߯?YÙÉQnÜ?SGMQ[á?fK›…G"?kš"xùWš?ïªÞ1é?m4®ßW8(?s† Ù*"?cîÙ †ƒ?wnSR‰ûò?aˆ£cX%?ïØ®""«î?f1|V2i?S;íh?ç4e$oÙ?s3p¹QÌ?f¥vcŠòAGN3FGL J1931.1+0937@GÍÀÓgÀ0î#;nÀ7þÍ;,&À:­?}ÄQ?É@-e²"@縨ã?ýà Éc·¿æœò1¾Ç"¿Ø?R}r¾Ü¿Ür£»Üdš¿ÖN—+™ûƒAGNbll?ï¶"8_ ?"<ÍIJ%?H—ÌãAcð?MWzˆ=?€ñžU"–¸?ƒPJ8éñ˜?î"䈳Ì?³R òq¨?'²ó–'ä?‰õHåù£Ø?©2´ÐZ4¥?°þAµ?ëmˆ»ó-+?±?^"ø•?šBút§|?öÌÍ`?¾ûƒª« ?¯PR
J¹?îi0®k?–"q›áŽ?Awæ'öG¢?Cm˕ü_'?©)íX@Zy?–/ÂF~B?ïôW<?TŒ<ÉêÜ6?3Êºz2?0pJBQßË?R÷r.Î?RëÎfË?ïGãh' ? yþ;Ý?p/õ)Ml?uÑ$xò?'÷•žv?œbÛWÚ%‰?îaE±a•?W7ñÊ7e?ŽŸ3{Fa'?‰ÜAT¡&ˆ?¢CÚB¨²k?–Ÿ\ù–‰Ž?ït5³ý.?w†Àñó²ö?9¶}hS+?-Ç4JkF‹?'úr¢^å?wJÐj/ƒ"AGN3FGL J1932.2+1916@KR ö½?¹†¿ÉÅaÀ7r?«ºbÀ:Rîu"Ó@‹1:Š•p@õi3JZA?ý"ò0±T¿Û ×æÜBŒ¿åÇÜÞÉ`¿êgž~¿íA‰Ï:ÿõPSRPSR?‰…Øw#?Œ5€Bð~?ä¦AÛÓ?Ñjù࣐¶?ÕëY§ˆ'?Ñ%É-¨Q?,~¿5{'?G P
"Ä ?ç=£ÿ?¿§0ùûŒ±?тl§©ì?¿¤c%ƒ'?¨±dêÏçë?›['&ê(?à'!ä'wx?ÁI~Ž¦K"?Ûŏ™ï"?Àð5ÆF²?t£ö»š?kÐ;ÌqΞ?ê5.ãÏô?°W/"Ûz?Ɔ,_.Ž´?°/Ó´ˆã]?yŝ‹/ø?‡/yyÅg?ê+vピí?ÊÞÔ-¶"?ƃ÷"9Ï?ÉT–
Õ`?HC¼¬9ø~?Yh$•'Q?èâõ¿EŒ?°¡†Aàæƒ?Íp0kÏÿ)?°ªD.$¢ï?²d$ËD?¢MœŽ'?â~‹~Mã¹?»k=TŽ"?ÖÏúº×é?»š%Ç:?}-³Æ"G?o(£™?6?ëÙ¼8CØ?¤nùÃ1	ç?Âã·¢¬=?¤ «¿]Ž×PSR3FGL J1932.6-4537@v
…@FA-À9ï)ªIëÀ9—*}'ÞÀ;©ôö·â¿ÜøbøGÏÍ@Wª³|D@ "À@øC¿Ú€²[Ìi¿ëbœ#P€æ¿ÔÑð֟çð¿ïÿí ²Û"AGNfsrq?ï¹u³q˜/?…Èb¸p?2ëàÌӔ§?9֎+ooE?4!ÖИ?…}œ++?ïÉÇ+DŸ?™­±W+M?:£×?å	=Æ&?–˜ESÃô?–¼h"¡º?íR¤¢·$š?¡a˜·¡‹?›'Úˆóò?‹xñÎüâE?­AÈοb? D÷Îê?î®ÀH?™
>\Ä?g²6[wC/?k¥^J˜g†?£˜ÛBb?˜*³ÀˆÝ?ïÑ,hœT=?…LÒEÑ~4?2Ý4'p'à?7õÕCàs?v;øoŽx?…3W®-I?ï£ÖQE?ƒ%T§dñç?kaÛxÊ^¹?iÅ0V£?€1ôÏ·A,?}m€!}?î%õ¤v0M?›2#ä›'?•öM¡3ñé?‰'îGìŠ?¢¥~ꖷ<?—Ô½#dóš?ï¸6KQÉ2?ryxnî?OÝÁÒÕ¥˜?G;:ì&Â?é"e.;?r"Ü0âˆAGN3FGL J1933.4+0727@F4^ FÇeÀKËè À9Ìò''sãÀ;K®æ1ø¡À47ŸÔq1@"ôW€D‰?ûäÛߏG0¿ïÿöµÿF?ïÿ°²Ô˜¿Ì/'ŠÒÓ¿åSd¹AGNbcu?ï\"¥=ß?–ÀøË[È#?aYÀEól?aIf=..F?'PsW]ƒ?•¬tèŠB?ì˜ø§¥Ô?Ä`ç^Ñû?'›â‡Ì?›ÉDf"0??¶òy³*?ÂŽÔn­?í¬¶ø'¼?›45H‡9?"x<@î ?…8ñ‡C
)?«+oçø?—OLgŽcî?ï[ôä;?""Æ¿ï#!?^ím*¡¦p?nðùõËXä?''—x«X ?"iD"ã	?ï´­é,}?'ð÷f?NìÐ×´ì=?M{nÖj>Ç?€å¸™¤ª?'Õ#)óú?îȝïzÝÓ?´1äË{{è?|y>‡\?ŽNÆäâj?Ÿæ|q ÆÍ?±(ßx ¬?îöç>¬ÒË?ŽòC&?ƒ´éËÇÿ]?uÐȺÛfû?—H£K¸Ôâ?Œv<VÏC?ïÏŽóg/?u(§Éûe?%¬Õë#÷~?6Eþã	?wÌQ»S9£?uØ¢†ÏAGN3FGL J1935.5+8355@]ÁÁÖυ@9τ´Ñ.À:9‡aˆ±À<£mWò/¿öxƒ.ž#@"£]'­A@Çó?Ó)³¿èž	㉿à+xÿ›+¿çCú°¿âÚ)nä9PAGNbcu?ïD .&aœ?¡†5×°ß?i€¹-™ò?uÃ.g?"Kã3V3? -Ió?Ý?ï'vWJ>½?ú7þ&À?v"H_}‡?[4""D™?€æè?‡³D÷'‰?íe1®+"?¢R'?¥_à?™Ç^Ò2N?ïùí€ò?¬É5¶Âµ¢? W…î"#?ï|Áу&?†ÿÇ(â¼?\)€òûªò?be=òæ?Jˆ±·??…¼!L䆾?ïo™¨)¡±?¶T˦øuõ?`7("V?Žèâqí?åóö?´¸3œ©]K?ïÛÎ8mëÒ?n½gZ©X!?]þ6Êìö¬?WXÑÓ£h?e2¬6<š–?hëÆÓÝ?îö¢§?ˆ
QÇÛ½?‡`ìdC?ÙÚ°Dë¿?•{FË«	?Œ~î&´?ïëáʓj?`‰'%ô´Z?#Y}ÿÏÖ?Íó<¦Âà?cMøàÁÁ??`NÌ"¤5ýAGN3FGL J1936.9-4719@uò®ŸðË°À;î€{»bÀ9he˜ºÀ;>`ñ—‡?Îí,öz'@Š+"+ÁO?úAÆa"Ú ¿êü¼Ëfµ?ƒPØ5¿2¿ÕÏ
ž¿ºhÿ{~Y*AGNbll?ïû–çì›?6)žÂŽKö?'™Ñzb;<?"†VI¶ž?7{ÙEFun?0ÛÁ)5¬
?ïxd—Hm?ŽS1";µ?nÒAè@
g?|%Çaù?Š2I¤íj?‡‹B'…?ï!=Õ¬"?ˆdGmÌ?†¤›ò y?|`rÙSÕR?J»A}?'¢~{KFñ?ïƒ^].?4{Uãk³?I>'
6Ë?PŸÓˆ"bú?ž…Ÿ«pJ…?֗ª?Õ?ïôbÿdà»?…4Ýç®"Þ??·™§š?p}dšëž?N˜5Ž}ÁØ?z©ë4
°r?ïÔóïÔ‰?qB:IjÛ?Væ†..œ?RÓtN\T?o™>°Ç`?lˆO&Ð?ïŒi®»â?pÖ~É ?y%šÌÓ
‡?tU³C?€RîñW4?{sþ'æõy?ï¼q",$Ì?hóm¶k?CŽû®J?<‰þö7U'?U|}àœ?h]ø¶äAGN3FGL J1937.0-3956@vrìà2ÛÀ9SÂÀð À8ÖϦ›àœÀ;y°Øzù?à4èß
R@þÚæëÝ@fë¿VA«¿æ-Råf\ç¿éÆ@ÓH«¯¿çA#5åA¿éó¨—´AGNfsrq?ïü6p:¶Æ?4t{JˆOÜ?)ÝÃÿ‡ò?%슄ëûÜ?1ÃUL´?+_ZNekõ?îòsÿ~¿?¢IKÚf?€‡¡å7²?'­˜^ø?™m¯,"7Ï? #'§ô'?îüûÖÇ?…](NŽê?ˆQèã«Kù?r¤4J½ò?"7¨OúE)?®ï?áÿ?íùö¾/GŽ?žÜ54:%]?"ÿ3½¡Õ‹?xº5Á'?« Ç*3uÇ?¨0ŸÕÔÐ?ïýÏ4lTx?#o}ÌöNi? "RW^!Á?&³+û³?"xh³XËf?ŽÍh{?ï¢Á†¦*?†ílíxšÅ?hÛÌ,[ƒ*?a±P]N.s?«E/3p?"}7ëE?ï…éq{ËÜ?q£Ž'ô?ze\±÷>?a±ºÒkI?RõVìéR?lwRÑüX?ïˆèÿ)ã¡?€yñ*˖?n•Y,dâ?X«÷¼¥èP?† iêÅÕ9?~ºvÕ꘾AGN3FGL J1939.6-4925@uÏ¿˜0äÀ;ÜLŸëÃ2À:5¢,RƒÀ;ŽŸ–2ÜÌ?éù·ê¬%@
Ý,µ?½Z?ùüÿ"µb¿î&µ´NÉ?ïþÖ¥œ9æ?žØh-Þ,¿äèòÂÕ¨AGNbcu?ïÈ®—Oô?ƒ3k¢ÈdÜ?RÊ]¨	Ò?`ïð­Å}%?vöþó£l?€?~š`¦?é<_²~S?ÃÜÀ_Dù?ºŸFþRg?¹[ðò'ž?»€¶¦U?µ,ÇmÄ'?í¨ôÖߨÐ?žº`K‰?—ßÁ¸ÅÏ?‹ÌÚŒz?©#´˜¬?˜­Ïï\'Õ?êùódCÔõ?»"Œ†?¶Ž9¬›•L?¶"âÿÞ¬?±¢+2ý'?¯.ÄÛß×?ïçÓžÌ^?mÿþ—9õ?>">ÃÖ@?L8Ǽñì'?d\Z…Çԏ?h¶)A̹ç?íŠtdÎ-A?¶ê?ʔe?¥Z˜:¿†£?²¨]þ· U?¡þ!uÉðI?žÔGÈõ'?î汏Ú~?':™‹ZH?Š—òpæ?"ÙnÛOÓo?•Ýì2Weù?Š0"…N,5?íhB½c?£ORŸEfM?®¹t´%? ©ÏFϝ7?•ŒX¹5³o?áëOÁI¼AGN3FGL J1941.2-6210@tèWÿ›V2À=…êÀӚFÀ8´wM>w4À;xv̗?íõíqL@§[-M@%@u¿]MŽ¿Û[-3{׿æU™ªû0¿åIUÐRN"¿ì)Ø`Ô¬AGNbcu?ïët©8§?`e‹üN?^júPdۛ?]É›oˆ?EWɦ¸Í"?;^çJ"7?ïLa¥axì?"ž¼'¿àÌ?u±'¿¡ÊL?_"f½']?'f¡€µö?Uy¼Ö÷?íòÎj ?›b¼T?£`î d€?"Ó"n˜N?šý!àAÍ?‹ìò¦ƒ?ïp"Mæy?•2ÚB¸(©?tºR-•«¡?uPWƒãÁ?˜ÃXëå§ö?"é,égï?ïóäži?VðÓÝ MÇ?SV("L.?UnÛa±g?9Òíµ›Ñ·?0SQCJ±Q?ïºÔÆQ™·?{òñèMÑ?c\'X)ë?^c†ÒSÞ?xç‰'º»Ê?vr%SüøS?îߥ3;þ?'b¾ö?—}Bî3œ1?‹ñߕw,$?‰>áœ?yÃAÅß~?ïÊyÛþ]?u–4ž³?`qfˆ>å-?Z	3ñD?rŠÁ1´"%?s$¸ÛUHAGN3FGL J1941.8+7218@ZÁ?ÐÐh@6ÀA¤À9]þÀdßÀ;Ÿö\OŽ?ó'-ªP@L÷¥¾k
@Z9¿¿H*¿ã•ó‹¿è"}š¬ál¿êISäŒ:¿ì–a\Ö¥AGNbcu?ï YšX¹Þ?ˆ"mõHá?+-GJ[?ƒË
aìÉâ?jù°¬ÄèR?p(^"3¦?íÝ~úm*6?°vrfé‡Ý?¢ê™ÚdÂ?šêoϵ?žzípj0?©?bô?ín@㨏?¢ó³k|ж?©Æ䰍3×?œ&?ûZ¹?žª.û!;?"k%®^yg?é
\2ìøx?¯÷"-›y?Âq‰žà´?¬#üÕU?²Ê9Èn[?¦Çt.ŒA?ïޕºÅkã?lŽ2£º[?k'rQä˲?ja;ç‡B:?G_KÉÅ¡¶?B'¬5þå?ïÏô@ül?™938¢Äø?ŽwÀ\Ð0G?…6‹Á˜%?ŠTB…2DÑ?"üÈr]8?îVUª™
?—·'¥Æªr?¢Ã	Ό ?"*¸g|™?5ٗÅ~?‡¯¬ü.?í§Ô§˜F?"Üð†‰?­C	½^"á?ÒáÍ«?iÐOÏ{?…"ñÙÜÎAGN3FGL J1942.7+1033@HÝ Y§;ÀuÈ@K·À8:Cû"~À:Á'h$¬ˆ?ïÃ|"jÞ@Š)åË?ý¦?Dc‡?¨lÑir¿ÒÛz,Êký¿ÝÍؚ$GÍ¿Ûܟ†K;ÆAGNbcu?êâD6vð³?µÚ–9»?³I̅\Ô?—usî÷?ÀÀ…ì"'˜?³Ì_kTÊ£?甕C¶õ?Ïh\çëY?°ÑÛ"§ª?³í¼RùnŽ?ÉD½`ët¥?Èa¸¤E?è2VË$h?±Š]ý¬×?°뢩L?™Hû؏3ö?Ç5Ü'z?¯Kv+Q§?ߏ¬§NŸ?±¢9»?²àÃ("!Ø?¥®"
/á?Û¸À‰P(ë?²<UMà?î.5‰"€ë?¡·ºKRÕ3?‹è4­ã±?…û1Nµ"?¦"š<__j?Ze®ýÎ?ëÀ´î‰µ÷?ÆXâÏîjV?¦vô½ˆÌ?²Aúøvw??¶¾Þ{å˜d?¼{Ö nƘ?젓
´9?¥Zœuð[Ã?£µY1­I?•"k痚?±qŒü{†Ì? "®fìY?æ	 äÖGº?¥\³1¶ªx?²/œƒí?"&~›œ?ÎÁ®-äY?£†ç
¶dAGN3FGL J1943.2-3510@ƒ/ÀÀ93_ý–™À9"ÞFqÔYÀ;‡^¼Mùˆ¿ÁˆÛrú?ï@b•ZDÅ@Â@+"-¿âÀ'Æ…z¿éèF>ÂwM¿â¸%ÔX¿ïÿʓ6©	AGNbll?''$¼?¨T1EøPÂ?ZéðGÈåæ?_áù&–?¥_®%BŒ?§ðh¢´¡?ëp"<jêZ?¸ØzM'??­~Ú¹[?©KŠ¡ã?µ¿%*?³–
è³Ï?ëZW¡}¯?¦/ºDh-?°!í"@Í?–"ÄÇ?µU相¶? ÉgrÂú˜?çÛuÎ}í?±£/ÂÖÍÙ?®&_¿?¢?ft¡¥?ɐÕI?¯3šC/!"?FA`{?'®âb"\?KØ-H29n?Jžÿç3'?‹•ë›6U;?'Q³}¥°?îWÖpŠ!?¥:QÒ´?"Ø»
''?4µ$'à? —¦c-?Ÿ£T³'?íñ®Õ&HÐ?–æ	Ýï÷Ú? þɯmÄ?‡2ã#¶?ŸÌ'ÿÌrm?)[''Š?íŠ_S$?•6Ö<y?"ÑÇ`æÅ}?ƒàƒøÅg?­o&]ʦü?'<()ˆÈ8AGN3FGL J1944.1-4523@vAà?pXÀ;ڙ÷LÀ:²ÕíݾÀ;Åëõ‡:?Õ¾°>÷Œ"@
MYÁ<uÒ?øô­ÿ'+¿¿ïSZðç^?Är0ìSr:?¸
K?eè߿ڔcl®KAGNbcu?ïí먧Ã?[¾²¥%¶?/¶Dîس?,"¾*áÊz?`…&`âý?YýC*€ÀÝ?ïTõWQíÖ?OÈúú?rÐCÒ I{?sWÆdw©¨?­D"Bå?ŒoÓU0?äãÖ?‰?·ÒŸ±?‰ÑŸÈÇTt?yø"8r?›c"€Ùaä?ƒn{y™,5?ï'uÿzbá?–CÀ‡	Ã$?`˜âm%¥à?g˜ Ý@'?˜þ#Äƽ?•Š¾&Å%^?ïõ†‡në?P4YÎ5
Ø?%܅ɛž´?$é³xÂþP?R7`ªäŸ?NYö÷Ôì±?ïÇCk?sï"Ó\`
?]Fò´é-b?U°yTá ó?u(¸ 
ó?pýȕÍ©?ïeðÛR1?z
£uÚZ?}Ý.ŸEÅ"?q"—âÜ®?‡•1Òv_!?qJâbDr"?ïÁÊ&÷ˆ?q2§»þðÍ?c‡ö祰?^pbÜu¹¤?uVñ2©›?iª€ûáAGN3FGL J1945.9-3115@!Ø,àèÀ8"ªKÀ9-Ë)^žÀ;kÇc€À]
ÐXó@àqŸªÆ@̂Ÿ­¿æ¦;r®¿è¹áaÅ¿ØÕ5¿åÍæŽÙ¢AGNbll?ïÆû_æ?{øér4Ná?b«gˆM?aÏùÿ==õ?s,œ¹‡<I?v—çڛ ?ïfï¶àë?˜Ýñ"´|–?rA§wK8ª?ƒçB"Ì8?#>Òpò?')ta¸È?í]gǏv*?ŸLýA†H‰?›«iàc=?‹/iÏýXÜ?¬SɌ »?—´Q<ñ$?î ¬y4
?¡ÍZ¥ãµå?'¯ÔÚeyE?6, 	‰˜,?¥ç^îà¹?¡ÄÚubõÇ?ï×ÝõÇ q?§‹6,÷TÂ?Lô7âÔi?LŽ='BŠÊ?prµËÌ?§Ž)¬X?ïËÏÕ¦÷?ƒaN)#Ôâ?[ǦÇ#pk?k¦áݘ?s®W´üZ?{•ÿœßõv?ï7)??‡oì`¶°?‡E n*÷?yWãM#î?'Jœ®X?~O}?ÒÆ?ï®%†'?}ÄL¡÷g§>õ¤/ï^@…?¨y4Öñ.?"kÌIt´!?}À‰Òb/AGN3FGL J1949.0+1312@I«?ÚácÀŒ,ºËCÀ9²A'è|VÀ;A'¡ Ï?àäß@ƒå"¯‹@KxßdÔì?ïÿƒ¯]·Q¿ä7¯JA'ú¿æÌ°i·¿Öý¾Û%3AGNbcu?ï¶Awý‹?…#kZ ?gëVC¼>ö?p	¡TJ#?xé˜þEÃ?'êuŒA"ç?ë{äZ£?ÆcPztmï?"¥›­ŒP?—ÄH	}.?¾Ú¹ñ0Ö?ÄL¾ZÕJ?í£—"†µ;?Æw@ ¦?™aœ%…¸¡?ˆž¥	HÚä?©¸¤ÑÏú?™Œ´®ÈÕÇ?ë'#6Íâ?°èºò]?†:U™îà?…¿ä©YÍs?ÀSÍÌ?øØ?°ŽB@?¬?ïâÆÌW±î?qmE#«?X®™ýâÚ?g—Ýãe¸?`ò\V¡K?i¸êj!	?î‡ó8
LN?­ýBx"ýÔ?0t£)?ƒjA̾?£@yŒ-×?ª'¼ÿ¦ô?)¢T˜?™òZ	\?ã÷]Z~E?ŠEO£'ù?iãg{¶Æ?"ZíÒÏòÑ?è/:?"®M«"K?v'¸Ò?kHéÒé?¡t@ú`?"Rn<¶ÞAGN3FGL J1949.4-6140@tò$ p¸ÐÀ>yn Ç‹DÀ:Vû…Fü>À;º%—i=±¿íÕµ‹"h@Œª^¸È@vý §•[¿í5}€¼Ür¿áÄ´ø@'¿×4#H.˜¿êç…-YˆAGNbcu?ïÛS꧗ù?mža¢*æt?ocmóh£?l=C!Ó½i?E"ŸÆ¬€?A—÷-üF?ïrúÏОz?d¤?oĎÂRƒÜ?€jÍQ¢¢?‹P(W$8 ?†Êäë&ª?îÔ.¸F¥?™Ø³:•å?¢
L(?"æR"ðA‡?˜±eŠ•½?‰RÝ~¾û?ïe£ú+æÊ?…ó¸;HÀ?A[ØŠ?B"VMଇ?'À¨2Uì?…êêS?ïìwñdlø?_Œ'6Õð?_`S*'N?[Ãÿ7Dó?>¿&×ô¿?:*á!lºÝ?ïӝ—S¼?p,ƒ-&íÀ?Ve› ­?RŸÅq}Š‰?p˜áýî?jÁè nq?ï.u¬z?ŠSôÿðn?'EÛöC:S?‡U'öÅÁ+?í*¶p¯?s¬å†Ä:?ïÞúQ?bÁ?]d/pV7n?+~¼†?!Çñ.Â$?oT†üqGÆ?\¥™"¢§:AGN3FGL J1951.6+2926@Pjå?õ¹U?õh?."À9R"狔ôÀ:é'üft?ö*åS×B@T+ê¿|?ôg ÈÍcÌ¿ßs©$Ññz¿Þ'0",J¿èrNÁÙÿ¿ï9ºHfOTHERspp?LmLü¶^?'åz8»i?ãÛ¶¹ÝSO?Ϝª
bÇ©?×N/!o€/?ÏÁŽÖ+Û?µŠ\¢³Â¼?ÀúHTœSL?ÚïòkÂƺ?É/ý¯ÔՖ?ß­vjë[X?ÊM*ä7Ö?É´ùf³¾3?±kÄz<ø?â7†IZ¼å?·C@ù˜¨?Ílíq»Œ¼?°I™`…Î?Ə~$jã?·''¦Jóg?ÞÏ=WæX?Ã':46ò?Õ閯ѷ?Ã-Í×Å?¡^bßZ?¨—;2AW?ãØÂÏGü?ÐNéøV¾S?ÖЌM3m?Ð&•¢ácT?ÒlĨªÈZ?ђùù	¤?֚úPØNz?ÇËm' "ò?ÖøAÉë?Ç/xJG*?Ù§\Åþ§e?´æ5dÌï?Úù6_Ø?±²¡zg
ü?ƾٵú‰…?«v
Ã.f»?Ñ~ÉÖðŠ?··öá½,˜?Þù'Lw?¸ð}HÙw?ÏâÒ]/†?¹ï³@;MIXED3FGL J1952.9+3253@Q2	ÀÂl@šñ`*CÀ6œÔÞF.À:›™[†8"@¯A"4Ø@'©«µz÷@Ná¾\¿Õ²Àe¡'¿á(ò"OhÒ¿æ{"噑¿ìèj"U¾PSRPSR?.–…Ãoî?)K•)ÌÎ?ïù0w/ü?IJ/‰Ê?C˜€â{i­?Ft–S?(‡'£ä¸Î?AœDÚ÷?ì<«õoa?µdŠêMgò?¾¿7-?µbŒzw??‹6·pEíˆ?ˆ|'¾1h(?íß'qXþ?›TJ­•?«?ÛéXÈ?•áðÎÉ!?MjÌÑ,ó?N"e:yq?ï4¾¾õ§??'è-ËI?˜|ÑÈñ1A?'nåèðð?,Cš‰•9z?,g¼07"?ïù¬`4Œé?J(f¼i?B=˜‹óÉ>?EÚ a[r4?IOUxHò?euÞj5SK?ìMÉϗWu?­™QöòÚ
?½_×jö?­xLë0´*? D6j*?— Æ‡Ùë©?í€Ë"céE?¡ÓùvU?§¯mûs8?–Iô—.´?[ë´Nê´j?OžŸJB›?ïE}å!ò?ˆYþôÉ2?•'ˆG@Û?‡\ˆÔëÎFPSR3FGL J1954.2+2836@PO­K6?؀ǿáp¸À6ó®«y•îÀ:QÏng¼¨@æa³Ï$ì@ÎC°.@»ò¯Šq³¿×$Á®"0,¿àËÁcj¼¿å xðÏþ¿ì…i/ˆG¦PSRPSR?;N}ý¥W?BFß;	¶?ïÄüøt×?"÷ô·°,™?{ÑNîxä°?"ÆÊïa~?3uj_;:?TgÉ®?éâ¿$ÃÎ?·€ðþ2ß÷?ÈkHåïU?·|´…Ï?ô¡4;¡?|enÿÈ?íû¶µ?¡êFHMq"?µ'ÝÂÝC? º1‡Æå?lzBZQ?eLηøó#?ìzÉs7@o?¥j(·Ó?»Hè•ïÚ³?¤s¶dŽF–?5½Ä•ã?@^b
ƛ?ïÇÏ–?"seD?z¼–}i:?"½ÃD5Ù?Pî$:×7?g¦«U½"?êxI_;ò?­!˜è* ?Åþ´¦eY÷?­,7€ÌÍ?\üÏ+ÉH?ŒÅ‰I« ?ìàç
À²ã?£$ê)°Ñº?µ
'ù̽¼?¡²‰ÐYçU?u$¸åòà?eNÛw»õ?ì·ZuJœ?P0@¥ç¥?¸òàǾ`œ?œ†QñÂÙPSR3FGL J1954.8-1122@=¯@Î&iÀ3(¿ó vÀ8d£zÃë}À;Oß;dZ?ó"ýèù~1@eSvŸ™Ž@+"ÿѱä¿ã=/!î¿âÝ@Š´¤b¿æ»j¥Bø¬¿çä¢WNAGNfsrq?ïä¤IB`š?f¸¨Â†?XL|Ú@È?Z&6K¯—?^jð%LÙ¸?]˜õnÅü?ï®™M0?ž+	{ÑH?|9«	"¥?|7ø_Â?•ûÂù\?šò;â¨X?îp[üñ®?"á'8R?–¡0ZÉvÂ?ˆæW>S˜q?›SlÇP!†?ŠYŽ3+rí?î-E4´ßè?šÓÛ´ÇŠ?';G–yùö?|T±ßì?¨œÚÑ#Fø?™Ð¨µ§}n?ï÷Á{£y?Gè-ÎFÙ??еUS9?>éK
p?A¹sÉZ†?=ÈøA†³?ï¦Y½Øày?†"³î73?g}öIΣ7?cJEŽ<2?€Šõôa?ƒ^´ï+4?ï;í°¶Ûc?†{_>Ka ?‰Žs¥ÞS?œ>‰…é?‡v =™/ë?xõG¹SÓz?ïr
Üë¦?~œ§Ó߉À?vËHóvË2?g7Xìá+?ˆä\±<ì?yGXnØ,AGN3FGL J1954.9-5640@uOº¿¹¾ÓÀ>üfß2*À9ø&yçL«À;¬&è¢i?ëáß͟Iv@Iè"Ïf?þ
•µ¢º¿ê³À;ÄÒ-¿æÙ~*ʦN¿Æ²˜£-Ž¿Ð¾cÓd©AGNbcu?ïÌÏViï?yQ÷î]q?B¬ŸB"ò?AŽ-&½?wBÓ³–Ø?x T»n'¡?ïXv—>©?Ñ™Ê­Å?p²v|4Œ*?l¹œ`¡¿ÿ?Ä~×?Œu×ü'8?íøIᱜ?*¯´–¨¬?š@'™Âc?Ž¤;y¡Ù8?£[Óò»?'qªÄ
?íóë`FøÉ?¡U€C"ü½?t¤"uː?â4ݾ?®>Õdâ2? [£1 s
?ïä"˜\ê?dì?ß4®?D+-éA´G??£"«fé?fa33?bsK"çwÛ?ïÉgä?Û?u!š8Ñ
?Zºv©?¬ü?S÷]<A´á?tÐ.qþƒ'?rL®ŒùUÊ?ï-ýº?‡›†zæ?ˆh‡ž‡y?{æð·¨e?ŒüŽø?zxc§Žáš?ïs¬÷‰'Ë?ƒŽCGN?u& '®Ôë?t[(œ`±6?ˆ±×.Ã?|&К¨àAGN3FGL J1955.0-1605@9 1ôoÀ5"
`:Ó;À9qá/Z`ŸÀ;^ꉯA¿à\L'ª@†Õûõ"Q@`=;"¿ßÍã}"S¯¿è2:àÚ(‰¿Ïñ¢Ål¿áû¶¡+"1AGNbcu?ï@í¿ûF÷?¢oÇ>;¦ª?c™½éH›2?d+g£"X?•o=–·³?¢2E¦Âô?î©	¨d&Š?­$a¾sß?…ÇU~1•A?&…E'¿?Ÿû /:ú)?¨/Ê­i®e?ìÐCÏ/? rLزx?œJ4@IRL?‰¦ID0uX?²kTv¾÷?œ ?YËè?êR¿"å`Ô?±÷ˆ5ŽÅ:?qñ*
{À&?s"CªŠéº?Æ%x_.Q?±õ"kWH?ïŠsòý_?™yz¶%?h›ÎroF?ÏTdÑÓ×?‡<‹õRc?"ýãí'´?sM?"ï͜šCÒ?o2"ïï8H?…În(Ûr?€ŠYÎ(ª?…´õg6@?î|S독š?•BàÇ¢ã½?Àünç?'b⯬eW? y[¡é?'§=vL\?îLX‹åÚm?'[#ÚS1Ñ?g,û-'?V·¿‰j9ì?©Ç§"Iîd?'ùƒäün{AGN3FGL J1955.1+1357@J^à€øÀ;– oÀ8áú"pmPÀ;6¬¯öÓ1?ï³–&@,ëp{é@é@kU¿ßÿ¦"÷@¿æE9BkàN¿á
ЬÅ	N¿éÓÇùåpAGNfsrq?ïÞc®XËý?hòÄÁ° ?W"wŠxÇ?\pT¾(³?eҕ§²7&?`Û%èãQö?î Վ£'?°réʒš?…]ã•N î?‹_-TOw1?¨›.1P5÷?­
`2!?îx#–÷Ã?™vÁ*츇?šâÑ,>2§?×'cõfØ?¡G0qj"?}ÃgWÚ?îÚnÔ&¼?"h<žN²?jZ ‡VÁ?kº¢ÕaÙª? ¸ˆçÓ?"Kð]³€?ïî"Ág¶?\d~&šø*?Pûc}CÈ»?Rw¨ˆ?Rû".§z†?M9û1jŠ-?ïF:·`ÿÊ?ž3n'·\?qøÃ1­Ëú?sˆ~y(?'ºx@ÁVÆ?šGÁ¼©?ï?%BÀÖ?‡
·>Aö?†éb{¥\?}¯ƒxù?‰Mªßi‡?|-r?﮺À°´¾?s'¯cq?cëÙ98!,?RÄž
Ä$?~¬³×Ä8?qNX¨'œAGN3FGL J1955.9+0212@E8"åx•À*ƒõž}.)À9÷Wfï"bÀ;o³1fª¿ó*ü6i@
œs]ð¡?þÖ
€·ux?ïøjb§ó'¿ãC_T	¨±¿â.­*M¹û¿Ó`óí»
AGNbcu?ï{CñO?$\šÔ?N=´A-:È?Kj{"6ˆ?K]ðw×?`îkþ·É?ï0J…Ó? Ç¸&QÂM?tÏÇTy¿?y;È~™™?"ÂýEY‰0?žOTlŒòÌ?íë-…Ÿ;Å?•&P‰ Ì@?"§—éS0Î?€J¸—U–?¦ù[³ö`F?'ñ#<q՘?íÛ¤ö£?¡»œ²T…Ñ?G§:÷žSm?M"ã}E?°øpüٙ?¡­²‡$—§?ïá5a®?p—¢ô¹1Y?8Œ'rŸ#ƒ?7cð³Œô?kÙðƒ)¥t?o>öŽ¨Öú?ïÃj
/?€Ýën%µ
?\,*I)w?Y	+sœ?w?﨎?‡¦¾¢gö?ïBX"ž?~ù"æ¯!?ð*	¿Í…?jsÿ°'è?y°äò…?yÜý+ÅAÇ?ï|n\mØå?€;X11‹?$>¿=?粓æã?INŸ(?€0É\dÛAGN3FGL J1957.0-3234@ "´ ©ÓÀ;4À_×,À9Åþ¦c¬xÀ;€­-¿ãAði\@s³û¼?@§Å_ÆB¿às¬ûԪſïþՇuC"?ï¯d3[L¿ä_Ë~GŒAGNfsrq?ïŸj\¦ZX?‰†»¤S?MŒ³±Óÿ?PÇu4/?†L'w'\?ˆ–*\ ?ï1NÆÙæ?£' O?iBè7?'ëßwúV?'ûàyóÒ?–.DsèÔ?ëåø¿…"?¥&­³"Ýì? ‡HZÎ?åõ€Ú?¸Ã{‡ü1k?¡çòÝ¡"?í–å©"à?¼5[Û·»?B'wÏ)?^¡^ëú?³*Ԙ\Ów?¼-‹tÈ?ïÎÞ¦DM?v§T¹.ü?;;«&S?DÍw¡ßÿ©?vàߎ{ok?u'ÿ!Qj?ïËu'[ë?¡><	rNå?o=ýû¸
?'þ½s]+¿?€½£*Q?™ìá*¬ðÇ?îGòèäÝ?–wíZ2'Ó?ˆ1¨ÝäŠ?yg¨7n?¥tSRk?"ô¡Ð|ã?öRF
?—¯Èµ/!?HDŠ@Y»?ktèJÓ?ŒY9Ô£`?•ö©çÜKAGN3FGL J1957.7+5034@U&¸`.>@&G^cb¦À8(ÂÂ#&À;täǕUg@ÿ¾Šêª-@ò/@µQÜ@—çZl³¿ÝŒr'¿–¿äÒBR5¿í;u-meM¿ïÿK<igÎPSRPSR?Š0ݤ}¦´?«û]Ò˙?ï2™"‰?²ßLN÷¯°?‰(à™¿Kˆ?¨É'ÚB3à?x^"±cJ?­]x ™h?î|fOa´?¶:™[¸?¬Ìi1ŠR?°£í6åõ\?ƊχÖè?®în1[Î¥?æÔψú÷?³I們¤œ?¼JÑä¨zw?£óe¬›î¢?m)ç‹96‡?nŸ"¥éß?ïy
ü;?ŒbÓFÔô»?ŠrÇŠÝ?‰hÝ
yË?'þS#c?¤Ø/g²Ó?îuµ¢sh?Àó\ä1˜S?ŸJø¦ä=©?ÀO<sxȔ?r[	/cxÖ?…q[Ó§?í•J'Œì?²+Ik'$Ë?²/þ—T'Õ?±ÄxgLå?Î"ÎB?±"0%Y"S?å87"šÎg?³[ÎkŠ?º6ÎïðF?¥†ñÉ¡î)?ËSU0–È?€•Šd?ï
‰$¾U?‰Œç
y?‹ÇJPQ?}åÇDJ¦MPSR3FGL J1958.0-3847?ø¿ÜÿŸÝÖÀ<úéŸkj²À8ƒêìÀ;GX&1Âñ?ö/R֑œ @ß*òœë@I1c$g"¿âͺPy¸¿å'¾7³ ¿çe"·'Üo¿ëxû¿S'yAGNfsrq?ïÛ'˜ö0ž?h¹¸ŒdW?iüPV‰Ã?eY"`af?U¸·žì¯‹?O¶æÒ¼ÿ'?ïsÝ'7ýG?Ž)T.¢Í?pPQëqàè?u'Ñ؈Ãb?Šà@gE¬?ˆ|Í6þ9™?íµx«7|?Ÿ¬Höä¯?¨}QÆc–?šM©ÓŽâû?˜e
Xª§c?‹/Ÿû"}©?ï‰ò}iõ?ŒOêZ?[p	ª/v?`<è?@?Š_zÉPÀ?‹3g5™??ïêDç]N?Y°9Ó:A?`s~NÒÝp?U½ç¸¨«ð?Eiº¨ž?;PåßÃÖS?ï͍°	ü?s*:†/ï?\©ËFŒÅ?X'˜òçÕó?rµ#/©j?n2<dŸÏ?î¨0f,ãA?"!ÅX¬lð?<xª`w?^'Mj?‹zõÄnï?? NjÈ]?ïä26*€Ô?p®¡ˆQà?O"0›{E&?QN³Ú±?cèýÑBÐz?n?צ›AGN3FGL J1958.2-3011@%åéÞU‹MÀ:Ǎà'ódÀ9×Ç.'Z¸À;h†`Ô¿©ñ/H;.ß@œ€9¡6q?ý²³?ê•œSÞ$¿æäWôÄɯ¿Â·è"cQ‰¿Ö|âž43AGNbll?ïúVãñ	?@ŽZëo?ßÇæˆ?jĨ1ù?Dƒ!x΍<??OÖÿ}£$?ï"VÔxß?‰'¾kð?lçS~ÒH?nKÍÉx	Ì?‡°vð'z?†­ö˜¯+?ïAxÌN"?ƒ¶´ý	?ï?|·,"ìÜ?i_ƒéÇ?£5·n•?W3T€‰Í?î›ý ö?–{ÇlRÉ?8ö©5U[ü?>µåâʦ?¦@®—?–[M×Äå‡?ïü4]C–Ç?5þ}¯E?‹C ‹"?
úqF¨¹?9ºFåP}?4f°ý4Ä?ïÑÕÙ¢‡?qŸqžÁ·?UíåS/í£?QöaþA?q™™Í#½R?nGÎþÞÖ?ï¢@¹¥õë?vœÔ#½¦?qBqQ?zw?_<åòn?}1â¤È?tˆ1ãÐ?ï­»ÕX·|?qÝð6ô?7ž–ã³í?,Õp;4?ƒÔï%µ?qžW&¬	AGN3FGL J1958.6+2845@PxèӔ¿Öƒ×`#¬-À7	.Cà)¡À:o9ä'\@æZSÒ@'€ÊjÇÊ?ÿWS–€	¦?<gºNoû¿à`ïë¿ç¨óºÞsú¿ë¬êŸ·çPSRPSR?U)çÆR~5?b"9ð¢y?ï®Þrí;?ŒF7ã?V·?£?/ùÁo?Š#õÜLÜ?J;éÞÀð?3¦()J…²?éÞx"Íh9?·Y‰à™¢?ȃTfgE½?·V¥Îè"A?‰åʗ	é°?ˆµãê/:)?êÒv[•Á¸?°j•ÜžòŒ?ÃÉéK;E?¯Ü8ZÒmý?a.!‰é'?]ƒ"ü§2?휸qdàï?¡b
}…²t?²'{Ɍ}? úÄ²?ZvÜ[?pa©ˆ
?ï²ÿÉBî?'ø‹>"¦?ø"‹HÚ ?$ƒöwə?800ÒõÞ?PC¡•Tì?êLQ"™?²UÓÅÍ?Ǔì7Ÿ?²YýN—41?£% Ò··+?›Få 5ó‹?ê&}¼³?®ô×)ò?œ Ù˜¦ï?«•lMÜò?m¡Ælpü?_µ™ò0g?í›$•zií?—·'zÖx?²9Í#†XN?–ñuÖ!ÞPSR3FGL J1959.1-4245@vQð€0<À=üÀu¦uÀ8šw§×IþÀ;~×¢äß?ð5b]]?@Æ&ö¶@Å»à~í¿áíÐGMû¿çB5×Ó;&¿æ`,,¦®¿ïn1–¥ôFAGNfsrq?ïñ~ í?R8øA·.Ò?I'Ï/"B?B.-ªËLë?QiÀñöË?J¨":îJ?ïo‰Â$ìã?=s³=ö?quþP$Ë?}ݏ"¿^Š?‹bU鏨?‡žÇ*÷P?îh=§¼ƒ:?'³6›y?®WV
4?‰"ÀXù€?•Ióë©ï™?ƒø+¾~d7?ïþªâ¹–?‡Þ'KR ?`ç€tô|?hóxÍ7&?"Fu6æ)–?†c0´¥O
?ïõDT?FâDZã?I øoï"È?@/	Æ'Z"?AͶQtq?5ð»#Û1L?ïÆU-Fo?vI
)§ì?_¿:pôɾ?[PÝ '$ú?tåšÝ1ñ?qTUyÒ|?îðžc¶fb?…2¯á¡É~?•¼:Í?
#ÌZXˆ?ˆÚ0ï~V?sro®ð‹?ïìa~¹Þ!?`r?
=Ü?Iºrç{?Eëñ¾1–V?Z»%«™J?\ÊÂå¥HAGN3FGL J1959.5+2047@M—ç@™ÅÀÅ)ÀBеÀ8¾í:*ž9À;2šY²ù½@)ï¶Ü @>2«#æ?ÿbxò)(¿Ò¼·µ}>´¿áæO̊Ìf¿é͉Ñ`Á¿ïÿÕOþ"PSRPSR?uv¯ž™?y7îbšG?íÖÆ̾Æ5?´¤®SB¥Ë?¯ïä[¸!??´×´©º?LIºCEo?^=a
5&?ê82ƒWZQ?º9¢&õ¦ú?Çì6¨]?º tÝ«?©¤NÁ_?–'ðÂp3Œ?ê«2wI(?©Pý'™M¢?½ÔE7Ó½?¤ý@T{NÍ?}Ò¦œ°?×vV	É?íA\êøÃ?¢"ÜwVüü?±Õ£þ$ó$? E,Žqr?uوӓÝb?†¾âj¾}?î…ŽÛá¤?°Ü-?Çé?«ìuôù¼š?¯ÌY»VYˆ?hŽÔƒ}?t¿áÈU›r?êYԐ̧Ÿ?¶òÛ¥{ѽ?Æ6rmZÌT?¶/d²â4?·í"÷:"?¢Œþƒ7´K?ê	©Ҋ¯?ª¿»ۙ$?·Å¬§PVÿ?¡œ¿¯Q¢?¥eHS1Ԅ?‰­Ë¥'g?ìªN•HÞ?›`¯ãµ?¯õÎPj¥?"·¹'Q°JPSR3FGL J1959.8-4725@uüÒ}ÔAÀ>Û'ÿùJÀ99ôêù¾À;D$¶˜­á?õÚÛö¶U<@9Üùë"â?è1k©,šÏ¿‡Ç·—¹ù¿½	[]ô§Ý¿Óâž/Ö\n¿àSݦ6AGNbcu?í½Cº6j?²Ez°
Ï[?©TÀzóª÷?«ç†K.Â?¦kG± r?¤!à•û ?ìC²å΄?À/Gb·|¦?¦'!4}É?­ÿ¨I
NÃ?´=QØmr}?·ÅrÏü
I?å¸vô~?¶F©p?Èuö&bjX?±ª_i»é!?À©£ÿñ^Ê?©×w[èD?å±½þ0z¥?¿®¶êÀÜ1?³wOí;Û?¬8Näµ8ì?Ï}`i@?½P%ò­Üó?í%Ôa&ó?¹{RÝàv?¨Kc—ßB6?µÑöZÏT?§?Â˧?§¦7È0j?îC%WŽ˜p?°¿¾:N?—»²£IÔ\?¡'n/'Î?Ÿß¢då²?¥bLÚ±äU?çãÍ·ÙJµ?´ÄZÕÿõp?ŀ))³Ç\?°îi°(ïf?µá?íΤ?¤'ÔïÖÉ?éžnºÃÇ?®çw]zG?¹j¢kÕZ?¢nÅOgâ¶?¹¡ç'­*?¦]W1B­AGN3FGL J2000.0+6509@X€Ì¿Ì3J@1ª_ÏspÀ7h¢q¯oÅÀ:¸aÏþ°u?¤âÛÊƬ@B"FY?þ!±á9u¿Ù¿Ìhù¾¿à2'U†ß¿Ú´Oñb‹ï¿Öƒ×¢¶PAGNbll?ïúŽšž7Ÿ?@Éše?${Y|Ϻj?#ò4;ÎÜ?@¦¾Ò·Dõ?;æ}[v!ˆ?ï™øG,—ì?º—*	Q?p€G#	'?mfˆûôú?Aêh0?‹i5VJÅ?îØåò¦œ?—ÉBZ–Å?'ŒéB.dÌ?……a~?›œÍk(	?""éÔRO?î[זTk?›jËuÀ¾¥?Gb¬ p•?E-–øë?©ògÙ0œü?›P?Îκ?ïýâêy
¼?'8¬ðVÆ?h¶£?KbÇI²C?'NY¨0—?"=íéØlW?ïÚÜʃ?t«;oÿ)´?Z&ó1'u?R+p²ÌÆÅ?hëª'šDƒ?rH'ñgŠ?ï#©r!'?"GÓ ç)?€,…êo/ó?dJ-ÓÔO?"tŽÁP!>?ÃPíÆQ?ï†àC÷ü{?x ~²Xô`?6=WÇIN?,sÒëzF?–€ç_å?x¾i¡ËAGN3FGL J2000.1+4212@SaqýÌI@ªE`zîÀ9A›\è8cÀ;!ÛjõA`¿òöƒ—¤¡à@ÅWìÐù,@¾3Ÿi½3¿ÞšXFú ©¿ã¨ž÷k÷¿êŠ"ë"çû¿Üö§‰‹AGNbcu?ïÌY²£Ö´?ˆÕ°.2:?aˆpðäŸ?`»° jíØ?qIb^>Û¥?ˆf/¸>N?¥µ??¨DÝwq›?vµùeôW?ve¤[&ßÃ?¤ðFƒÚÛý?¦Þê+F?í¬½SÄ3‡?™›08»Q?™ú7<À?ˆžŒo%
?¨76®Ü°?"®cLx?îHåä˜<ð?œdç̇¡'?K'44?Q"!ù´Z?«âc?œAЧDI}?ï3
Ú¼?¾©1è‹«?`×Wýk??‹êlgSÙ?š>³ƒ j?½ˆ®²&û?ï1njR?'Œ0p"a?bÊ.ºŽö?c^"ñõð?‡A2¦û"Ò?Žµ¸=†ŽÉ?ïTჾ?Š›«]4?ˆš nŽÂÀ?}úïÌ3{T?'h™øªš?ƒë\Ôfõ?oI?u }š$Ðå?"ÇåÜHÀs?H[™NÐ?‹ŠE}Z?u…3¢·TAGN3FGL J2000.4-2926@'Íä ¦hµÀ:ÿyŸÿhÀ9WMî \+À;jE­‰:§¿Õêú†÷ß@c²åE°@ÕúÁ;t¿é†pÞÓÇ¿æÞSèO¾¿ç«v-ƒÆÉ¿Ë1Æñ~YAGNfsrq?ïP†vðÙ?±Ø<ñ¼µ?f¥ÛÀpS?pAVk'i+?"uÞ9ÂÖ?±¯ÀºUµ?ï=Qôw?›ù8ãؚ?vñ:óô?ƒåøVŽ8/?'Ï¡ÿžÐ?–ÓҖ—3?íYrèÞXï?šüÁÒµÔj?žÛú±d–?‰ÛU
Òv?ªúԍ¾Ç?"h7÷¾?퍷s°b?£SJà	?dÞæ5½?kexz?²ð{j½…?¢Í´ºmŠÙ?îߪæPµ?Æ´]¦_Œ?Âä;´ý?©œ"áÿ?›)—Æ3?B?Á"*CÂÄÙ?ïÃH'áØ^?~ŸÍ''»W?`èBûÑh?dgºUrÒ?vNÊsHT?x7°:?ï™Ð(Õj?"UP}²?ˆÞ™}êçj?tÀýáBK?yBÏ?¢ ¯/©v?老ïz;?|šœ§¬³þ?G¢±.ҙÂ??êÿÍj?Žœ§§4þ?|XS$~ˆFAGN3FGL J2001.0-1750@7ýJ€àÀ7%A` JÀ8…Þs¾=¾À;G¯e³¹¿ÙLAþcXü@¤Ð.@z+µ—Ò¿â@0œªñ¿èö‡Éëúm¿Úê"65ú–¿å"ì0•IAGNfsrq?ïü}«ÄÆ?2iȹÝåh?ßÊlÈs>?UT¬Xÿ?8–¬+⁆?1h]ðc'Ð?Q{a?"5'tfx=?n0sª
™Ñ?€#6ÖøÀ?‡N³5YÑ?Œ°â)Žm?ïÅl¹Å<?‡e$>pš?ù ÐHš?p–Çz¨?–JÁýã[Š?"E
xÕþö?ï¬Áðáæ ?|®(RG¶#?K¨…³Å?o€Å#}?"žì…Gÿ¨?|Œ'h)­?ïþu'ÒÇ|?wCsÝw?L9+í7>û,o~h	?#"Æsß?POgœ°?ïÖY¦Ãy?oB'Öï«î?UÚáñ?SŠŠaˆ%<?n¹J
N†K?h"Ç3n	#?܀?s¾Ó=ÀÝ?s²ö2†ðâ?f\=—?€€¶6àH?nˆ4óí?ïðw,Ãh±?TuC7³»?B[=e8>þ³Tƒ¦º	?^o'pEÜZ?TcIÓj+AGN3FGL J2001.1+4352@SÄŸê³@s•À8–À7Ô¿ª¥À:k$;H«?ÓH îÀ›@T/(6ªâ?ÿŠsž³3ô¿àù ÀTnl¿à8îCȊ¿Û:K•Õ"Ç¿ßÕü#°AGNbll?ïîtà?ŒbQj'?CŽ²¨d0?GyܨÕ?‡…Öò3É?ŒBtŠ9¬?ï6˜£­ø)?™Ö¥\©à?q<ç]Í?p/i5÷³?"ݱ¶Ý)?—½GŠtK?ëjT8«1
?¯r'G?—›`7·Í?'Ùź§Ø?¾Æ™#tp¸?«Ü汋Žû?ï&þ"Ÿ%?'ªýµœd?+Wd†Ë?1Š2ʍ?šé¡Ø?' jR¶¨?ïðĚ	'6?[·6—$¢?*Ã?Ä·¯?&µW|öñ?[dhæš?Züdߏ‡q?︱@ Ã?'ÂDFJ£ý?]Ì?¦a'½?[MÇãsÍ@?|4Oìë
õ?€åé|¦†Ì?í±P72­?¢³âK99?Š;ÆñÍ-?‡_¢ÅÜ?®\
ô"¤Ù? ö¢‹À	?VëÂm?qÿ"Q¡?"@¯ïöþ¬?Û\5v¶–?€‰B|øh?qö\oÄí[AGN3FGL J2001.8+7041@YÕÑ_ÄÖ@3õÕߛªÀ9‰´	‡h?À;""²Çì?à̈́ò\@
‹oK<ih@§`¥aÏ?ïŲFŽ¯±¿ä—¿iÉ¿Õˆ&xqi¿â:&ù$TÚAGNbll?ïhRì®`ó?œ@,èVÆ)?w
85üL?zž_®ë«)?Šf(¶ª?™ñŒqSY?íp3é³Ú°?¼Ó½+ïòí?¥FsÍoCŒ?°¸^)ŽÁ:?£¶MšÂ­r?±fqÆcHœ?íÎU3²?šqë7˜ˆþ?˜Â¯žT?‰Ç'¼ÜŠr?¦½fÙL
Õ?")R‰º©_?çŽO¯H`?¹™²¥üuÔ?±ë²	¢Í?¨²l{ã­?ÈÐè>²<?·‡p®ž '?ïB|	÷áµ?½úÀ»q…©?c´ßKy®?i!‰fí\&?•NH(2?¾Æ
®?ïzG*D?¨¸§$<bk?øôA1®?—Dì,ß=/?O:§{'? "?ou'y?ï%ÁdR©µ?‡c	=«þ?†eï'ã?vøà$-Ì?|q1õ?ÃhJnD ?íbêl´¢ù?›ùé)hè?¡Ou›þò»?ŠÖ(z¤_;?¨ã•GA¶?–0	 ŒAGN3FGL J2002.7+6303@X
FŸ÷¬@0oò ClfÀ:i¨+,ÔtÀ;á|lb(ê?㙵·÷'@ý&±ÅŠ@#¿¢Â¸¿ä¡?[pz¿ìÒu³?ÀÔjÁÑv¿ÚsÜ
­XAGNbcu?ï櫐gä?q&ùR·"ó?&6£°ƒ5?%¹V$?Ý?gó,16n?qâÕaÁ?ï^ÐéÎ ›?•5ÓD·ÊD?uŒV,_îù?tݱªg19?…šm°ÛË?'‹ˆY·H°?îÍÝÓ|¶¬?Š*²b¶õ?"€µŠ"ÿ?sS`d'?œêËYgø?…Ùñ¬ä?ï Ips?˜Ò˜tÈ­B?g¶øï§Wœ?~Êùdb²?œ%pÉñÅ?–6JoúÙ?ïôɄTL?Té[‹ˆ_?]·:'Ü?i(o/?T—.t‰?TPŽy…X?ïÐîÊÎoå?yþ•õ£Ú?_•s›‹gÏ?XN\'Ÿá?oF{žã®±?wTî¬?ïuÏUpÓZ?y‹Ý#s*ý?vFÈ+Gjn?fLÚݹ1?‡hƅ8x<?sˆ4߉&«?ïƆR¦&V?uE–Ô!¾?f¼rƒ t?iS µp{o?q^s[ªë?i8_»AGN3FGL J2004.8+7003@Y¶Â!y@3téÅ+À9ò	7´À;‹ ¬Gò?°Ð®q¬x@ÏÇÓé¢?þ©€Â]2¿å÷\UÉé¡¿â§ÆZÂÄ5¿Ü¼»ŽrÊ¿ÇâzwÚAGNbll?ïù8W#A<?EÀ
wc»_?)Ï"§B?%ç,Hȉ?Dºo©uM?C{´Ï???ï®jE»mv?"Ç?OØ?n"M¶*?lüñØ÷ß¿?y€œ`	í?€5+Ó\¥?æxi?zþÁ‹ï÷?t
6¹¨?fŒq	¤?'Ñ<Àrí?w1¡ïZj?ï}¨Tûãn?€s4û]?A¥-t¼]·?G0å=`U?{—Üó9?ºš²~°ö?ïýb°h,?2թ̯H?#
¥ï,?%iðZÚºÌ?*ýÊñK™–?(8è/F?ïá¦2Úì?i´Òʅ§L?Wä•cÒ~è?S"¾ÎQ£?bg'M~4M?c®ØP?ïÃÀ_Š»?l«šhB©ß?iòDѤKœ?d1†"¸2?q&–õÖØ~?b$Na¦v?ïäã~Œo\?\f)'‡ ?3)hdWÖ?-"_foåç?h·T])ò²?[qΨcAGN3FGL J2005.2+7752@['¡ Ï@6¿¤Ÿ‡dÀ8š°hÀ;~¹Ù«?ôÍJtm@Ët‡ff;@¿Ý¿ŽJÜ¿àã?˘¿ãÄÊPà\¿á©ðìçŸa¿ç¥eµ2ÒAGNbll?ïñzðÐÑÙ?V™P‰0q?P.4í2
?RÇ'œ?I·ÓõböÆ?EˆÅÕ'
?ï¤G&IÄ?‰èÏ·¸¾?q'»NBb?o}ã]…|?|I±¨Bϔ?…‡œP¥?îØÓK'?'C«úëª?"÷×TŸ›e?‹2ÍyôLh?íÇþ¸[?'Hè<ñù.?ï ö‰x~?ƒâ0ú…U?bJ<lvô?a¼	uX?ƒ/΃Áû?ƒM¼ÆÊ?ïùê2Y?Aðq}?A)Äß÷3t?>#֐?,µÊ…Äm?%6¿²[ðx?ïÛà'ƒS:?ju»fÆ?`'¦#ÇÛ£?X¦ea.?cœÈHfʲ?cғ_
?ïaþºÛˆ§?ƒ'ص"£?†…æü%?|ÌE•ÄÎ?qÌK³ë?t'ÔJdé?ïåÔµúMd?g@[÷äÞÕ?U5Í×5ÉÍ?K§Ë¯ðî?_ ÅÀ¼½?c×I¦`«AGN3FGL J2006.0-2311@2ø÷àvͽÀ:-Z@¾61À9/?ÐÐgŒÀ;}|Ùor?îŽ"é+@hö'äöd@ö?ŒÝÉ¿áØp+â¿çrDoè脿ë™IÙõL¿æúÓÓ§1ˆAGNfsrq?ïù+ڛ¹Ò?FKÅ+ük?8(©Ð+·0?3¤ÛÄü™'?>x€F×Ox?ASäµ¢‹?ïZ;G?"ëՎ'ÞC?tH·cþþ?}†)èð8Ÿ?LÀ'ÄÒÇ?Þi bȍ?î¯"fh?Ž,!ŒÉF?ŒâãÛ¤?}±F¢ç?™Œ¡úÁF?‡ÔºZ`G?îóqªoÞ=?—Ò¼uÈ¡?x¹›y@?u©ús¦ÑH?›ccÛ$\?– ^Å2N²?ïüqQjŊ?0ú^nÿ??)€›äÞ×e?"kqkƋ?/jJf‡+f?&$~ìOe?ïÉ ­–?u‡9ð9­?_)GÞÑ0.?V7pƚæA?s¥W—[pÓ?q´pdµïã?ïV	2Èn?Ô†ø}ºÌ?" s9FìM?w«Ìû¦?†]@ L=Ö?wr%;¦¤?ïÃÝø¾?t€ä¸ò€?dŸÒ=YÆ?Wǹ ž¾@?sÁҕ>æ?q£–Ê"«ÔAGN3FGL J2007.3+6605@XÏè?ïÚ@1n´_î}!À9€ú:þÀ;'-±2ã?ÚQð"
yÌ@VÆwÉS@·ò ¿ãn×Ѹ™å¿ê°Ïb «¿å0Ì6àøå¿ïþ•2ñ]ÀAGNfsrq?ï÷bE«—?F·ÑBg:?:w(²Ê8?8óžz®aÈ?Es-Á#·B?@РÆq§¥?íüE¼*pÊ?¯ðµ<ëÌJ?š¬àæb´¦?–}˸_2?¢å3Ë€?©ÚQm ì?ï9D;»?†r–£Ú‹?'f†'÷§Ó?€nË÷zy?‹d¡àÒø'?yã8Lä;?ì+¥ý	«?¤øh:‰»A?¨ƒT[<ŠÍ?•Ýæè'UQ?²a%çáŸD?¡ ¡ÜÅO?ïûW£L?7¡æD½P?5.>õńƒ?1ù·ƒB© ?0¨Ûj?&—éCݾò?ïS.Ý|â?Œí"}j?"xv—¯Q?vÚÏïiùO?†»Òž·?‰0)Sæ{?ïc¿é ©??vÖÝi¡ˆ?ˆAí»M× ?q¢æ¸>?}œ/´@>€?aÛ«]'µ?îêâ'¯E?…"Î0zO?'Rk¡}'?uS'Ø®?'h¼_ŸÖ?'€t]`µxAGN3FGL J2007.7-7728@sË/ŸËÀ>Œ6`]'À9sÔöfú
À;›wï$æi¿°áõ"x'@ÿÀ+©§@výòÿf¿èz'V?ñ¿äòu¥Õ¿é¥þÓôÎ
¿ïÿ?9!AGNbcu?ïõ>âؖž?Svëù€?A£^èÔ¿Í?DÂ4F¯?Iaú¢p?Klå3Ÿ?ï*'•'ø\?"Á¶o‡v?x>°Æú­?xoŒ…¬ù?"žHã›0Î?'ê¶-(K0?îJµij
 ?–Už±Ë-?¡LaëH+?¢¿
¬?"U¹?†Õ´ËûÌ?î‰?Çô©h?›¢õ¸ÔG?ƒ²Âz~­?ƒ7¨<‰E?¢Rß_œT?—¶ÏNK+f?ïú-œU?BààRU*[?7_€î"AŠ?6ݦ9q	è?8ãË?5W}öIg?ï²Eôšµè?€jW²ÒyW?e/Å
½b4?`yh&Pÿ?|E#*f'Ù?{½«/aÎ?ï! æÌʖ?"äfõÂ	[?'è#݃=?kØ\þ?ƒç~•6|w?tß`®?ï´å觟?t–àÞ\?^WTtÔAÑ?TtAô«´?~h8³°?súWk%AGN3FGL J2007.8-4429@v6Ê?‰'ËÀ?ÕŸÕó½À9ŽTEÒr(À;­†Q¾8µ?ÈE'² ¤@F´šQ@¿œÿªšž¿ã>w"k4¿æä,J
æ
¿ë:ï.˜ç¿ÙÁ6ÓÉÆAGNnlsy1?ïì/MËdî?a16­µá?Ks*ùž9?PÈ'CÈK?YÙªm1ʾ?XDH&ÝÖà?ïS"¾é+Ë?—à'Jœ­?q7/³I2—?~fˆ÷À(?'MÜ645
?""Î(oõV?îÆüÌ¢c?‹ˆ²tæ?v½</1ü?€|ámšm?—e͜?'´"Y?îràn"ø?šØ	?tÆÃÞBo?uG—'Ö1?¦9 ±F °?šŸCm6;?ïõâüþ²'?QßJ»«‹`?<Gùws¡Õ?AªQt˜›?JP¼¿Ä?Gwî|óÙ?ï˼nŸŠ?w?"ÌIö?XtQœ?S}áĵ?tX
zjhú?t"÷8²V?ïyíî@Ì	?{Ú&óxùâ?~iÑø':ú?s]  Ý?'O›ijŒB?pÄÂnz^!?ï¹L‰½ÐÓ?u9ȒoH?RmMy9o?G¸=+µêS?~¾gÄáL0?sît/ŽAGN3FGL J2009.3-4849@uæ
 '§À@LZ&–mÀ7ӊë€ìúÀ:©³%[Ú¿íükl@@€¦Kٝ@?ü_ãìŸP¿Øfû"¿h¿ÛvÞX»X¿Ö2ä%Pi¿×-	þ±vZAGNBLL?ï÷j†[¤?NF–Å>ø›?ÖÂۀt
?|žçú?Pa¿&Ñ&o?MÂ¤ê ¹?ï"@–F?"G{m?bõ¨–À)?dÉk]F?†'ÙQÎ%?y$:'?ìòíOúW?ªÌºxúL>?~Ÿ›¥Þ-?ˆê°"[6õ?´Híš!Ô¼?¨(ý¹Ï{?î¬CÕ9ON?–ÁšÁA;O?"$ht½?Èey#{$?¥2±ž—1?–¾W)Œµ=?ïý4¾×Â?0E†Tãd?}"xO÷1?ÃÓ1#A?2`jƒŠ?-"Ø&wÒ,?ïÚâ,cý?j"†@\¢©?QißV'W?P+ ¢¹\?li"¿?eãËék?î¨-oò?—ßÂ^9N?…üM¼?ô€'[a? 
_[|ŸÛ?•;cb¸Í`?ïŽ*€J?u"æU !?¼4¹"8>ýõBŽ
,U?Œc£ºñ^?u'	
)
1AGN3FGL J2010.3+7228@ZVhÍJ¡@4$WÀ±5˜À9`¬é·À;Øwûº ?ö" =͕õ@Š•DË6@£3ø€ñ¿áí¬¼ó!1¿ä+ÚûIóû¿å{ÿUò6$¿ëêHeì»AGNbll?4ò?¥ÅP0ãÛ?£ZÔ–?£sRôH۟?ƒAð£]1?ÌZ-=eê?綤o
¤Ê?¾«ÿ"§fƒ?Ç_µgð?¶ìÝ^í?³Œ¯Hí?´Bº¾ Š?èuÉ÷
Î?´":ÚÇa?Ǩƒ¨|Ǎ?²C­.ðÚþ?ªQó>…à?˜çH ™]?äjÈJS'«?°—\~Î?¨?Р0«o?®I|ó1¿?º)¬ê·Ìé?¨ùB@œ?ï°vÂ3Û?€"""0‰d?^áñÑÛ×?Œ`
@aB?TΕjó?NÖÑ©]þÈ?ëŽ>áßzò?±Zbµ/a?¸‹lüŸÑ¬?§nãõµh?¦7çߐ?¦uF'Q‰¨?ì£-¼¦¹é?¥',Rb[;?´…¤ó쀯?¢7æg¦Íø?™ƒ´žæ\+?Žïh]U~^?êkçe`?œ~IQÅ©õ?l¡`YÔ?"gïÇ[pU?ÿ®W‰[?' C 3AGN3FGL J2012.0+4629@T"GŸÑÁÿ@ƒ32ÚÀ8PݝÕh}À;<äŒÜóÀ¿Ï+šã@Œ=AT@@Ü= ŸrL¿ä©‰[¿ã÷Z4,¿Ö?H=9$¿ã0I'f2uAGNbll?ïÞA—'›¯?tÔýÈk1Þ?!9m•?"0Ø*V¯è?pV³:‰y ?t+ªÐé?îTäã#?´ìʁä‰<?v=·6ƒÊ?
ދR7g?§÷zÍ×?³í@>¯IK?îŒzªÊ?žÎzqÂ,c?ŠÜS´sä?€5¿¬â!w?¨ÈÒws¹g?›J&Ҙ6ð?ïC?oN?"ÜD×"û¨?@/]¥¶?!qK[cN?—÷òNîN?"Ô«ÝKǕ?ïöÄø'`?Qæö]åG?Lï$ôî?ƒ)¬£0?PÑ@ç‰6)?Qqø«üv?ï'WpG¼?™æèèóZ;?bF¾4ixC?nñÐ3ߺ?†Ø×+©?–Ç-j`4ã?ï`z¢>D?"³ŽË®?x?ÏÚ*|?nQb%íƒ?‹Áȟ²£?`R^ERi?ïÌ˓Íãß?v-…¾€6Ò>ÝØä*FZ>ç½xÐ
uj?y'¿ò1'ñ?v,n±Û"/AGN3FGL J2012.1-1643@:=ÓÀíÀ9)?O¡(À9´a¼æÀ;°}À?`?û+çpÌ@¦5þ¿Ž @æsžg}¿Ò&ÞJ<}ù¿ì—ÁÜȇ2¿ïôƘw§ú¿Ùú39Š²˜AGNbll?ïŸ?îWŒ?"õƶË=2?vTtù¢È?"èHÃ6?z"êôQ·]?ƒè º§ˆ?î_yÖ8cý?´_|ö_h&?ë)`ïG?§&´7bi?¡'Íèú¬Ž?¬Ì\ƒq?ää3~»$Œ?¸Á‹r‡?ÈfÑ·(†î?²}üK%Ôa?Ä`Mêæá?°xL`vzj?êÚ³À6f?½rm'B0ž?´>«¤mŽø?¶
,!ó¥?·B~¿H‹Ò?³*[÷ú,i?﷉§ÄU?'Y†lÛ¹?t¼–­ƒÁÎ?†R¦ÿx?nýÊ%Ÿ~?"ž•4=?ï€Øëy?š}¢nߙŸ?r7HmajD?|ð4Ìž–?†®*欞Ž?•'9;E?æjtHëñ?µØRS>Sh?Å(ôâ&•?®ÜeïŒÜ?Á.–-ë$?¬?n"?î4j˜'?¦c´Y‰?L?¤`tË38Ÿ?¢š:ÁV}ä?±ÕQ`ä?Ž0©ôŽ:sAGN3FGL J2014.3-0047@Dýžà*w£À2ºÜ fèÀ9wU4åºÚÀ;Fù	q?Ø&‰åz `@5dЏ$ ?ýP!?Àµ?ç]G¦²±Ä¿áÙÅ(yØ¿Óè}†­G¿â'²Íƒg9AGNbll?ïû·Yr"?4!°z
«?Ði×G8?]A3	Í%?9×¾'ÔHÌ?0Rs¿úÄÐ?ï>·'.ïŠ?™A¬U…ƒè?w©vqy|‡?v(ýD¸?'>°9Ð"›?–²ÂàdÚ?ïKmö
ôñ?~áeídä?goíMÏ?oKçè¥?‹½‹Ü?wk+pÝã?ìáJ¥À™c?¡éMonq?oÆx'&{?i¶ÃÅÂåi?·÷z¶Aªv?¡"Ýg'@1?ïü\Ã&T?.¢´ÃâRÉ?!ê<ÂÛfˆ?+*ON?4$Éül©˜?%ò¢"‡ÆA?ï­_.cÀš?…òu)ˆ·?dÚ¯#?a˜›ÅÖQó?~ã\OD'?'ßu:?ï¥vêš?n¡.R""?sÑO~é?ax5R;›ë?ys£ðóc3?g2¤´')?ïÙ®»?•¾'ÍR?iئ›š"?U«ð?™éȹ RÏ?€UVÚw:AGN3FGL J2014.4+3606@Rw	ÎÒa?éƒ9õÐôÀ8íaö•À:i"ïQ0?õ'2T»ï@xq5¢NI@0~ÀzY
¿à	Ç^ÎÂp¿ã­¬`›¡1¿ë>H:+tù¿é&¯â[TeOTHERspp?€Mqï!ޒ?†vøž¦?æC"÷•Æ?Îyëz8±?ÓG
G]®ÿ?ÎÛ²nZ?'¬Ï![b?¨îóà"\?×¾îêÑ<?Ægÿìgzk?ã""€c›?Çz§™•?ÉAÊêcOt?°<ŽjLÇ?ÔCl2Є4?³P?i&©?ß®WýÔ?¶ô–ͼ?§@úQ—?Ÿ"¤7;Ý?ÝA1VAß?Å3Xr?ߘ¾0ˆ.?Äo^&?"W¢µ>i1? àÖ¬åõ¿?椾"‰{?Íí¥o?Ñq¬Þ7?Ì'e HÓ?¨°6RÈ0?¸@e½ø]D?Ö+šx«|?Â¥¨$½?ãj/P¿O?Äÿ´z4hV?Ü$ÂLì?µPœ‹_›Ñ?Ì÷Sî–L?ªî¹Cž‰o?Õ`TGÄ©'?´a³¢çó…?°°W›ÿAÃ? Ó"͏7?ßIV;²þ?º¡"_Ë!?܊"ÝÒ?»
÷~@«MIXED3FGL J2014.5+0648@Hw V·À.€LÁzÀ9o>À;T' ¦Ô¿Ú}ôÌ_‰@fSvt¦p?þ¤®àþˆ?çW­ËÕ¬¿èU‰%û^¨¿ÓïKº
ß¿ÙvŠq™±~AGNbcu?ïã™üÚ d?b°ÒÀ^®Ò?4RٟsS?.›[§È?iÛÁ
焝?aÞQÂUW?ï)øD{? €½iR`?uÐ&iî&?t^ ³?•LûvÒq?¿á¬Ø»˜?Àà»?r"˜/Ö?N¶\Î?{/[ù€(?ŸÎŠ†¯œ?ˆ7‰H=?씤š¦?¤•˜×"?VJ£)ÌÀU?Vº"!EÜ?»´àòɌ?¤ƒCuXnB?ïò¡šïÚï?L&ñ³× ?1ß»;z?)Å»fY|í?VEý÷»Y?Hî‹"S\?ﻄSÈeE?ƒ©j#_­œ?_ßÄ_?\A˜"?zxµ™ƒÙ?šp(/3?ïm?t ]Lɼ?~}<ÜRž?gal‹'hµ?…€àC(	?m5?†äo[?ïü`°'O?ƒiÀtõÙ?JÌg¸{%?=;œj,º5?œª¤êz?ƒ@b@pïAGN3FGL J2014.9+1623@L®¡@W%À$;ÿwDÀ9Õ(X䝤À;qhµËÿG?ºâÌÆö&Á@%2?@G]Ÿmn¿å‡'(Ap@¿æQ(óØï	¿äýt½1­¿Õ¬s¦jãNAGNbcu?ïC(ÍdÞb?šè?ù»/?jºÇûµe?m¶="…?²?"Cvà,?™±Ú\Ä?íÞ¼£ù‰?²ñ3ã¡z?‡qîÿ?Ðä1ãêÛ?¬Bµœ‰­?°"_éîa?îšyØ?•÷…Ë"?•ª8aì?'Ú-¡æ|œ?£°©9K…w?)6¶ô"þ?îXxæVò¼?"FÏ× ?d
"—îõõ?eB5ú-C?©7˜T—~Y?""uvlš?ï×ÖgoÎ?{m0Š*s™?Q;"Ühœ²?Q_Ó6â¬ë?o‹Íà¿d,?z#;‡(G"?ï1¶©IåÒ?£–]±ÙMÜ?sõj‡Ö¡)?2²É-=u?"ËÐ.žQy?Ÿ"ƒºf*?ïcÌ#•Â†?wÞ6xUZß?€1·<'²¦?gïNü@C™?†Û?ëÎ%Û?qjÒ¹ML?ù"L?s*BÏØwÕ?UÓRxùá
?I±K{?…œ²Óæí?rE$E†QPAGN3FGL J2015.2-0138@D§:¶~­À3XhÌÀ9%¹˜<¢HÀ;^||R`ö?ì8_Œ¤àí@
Í,݃©B@7* ís?±F(mÝS-¿åð"Ò.­à¿ã‹ü]¼§C¿åRÜN[>AGNbll?é}±Nʛù?½2ϱ¿¼T?¬Eyw^]
?¨‡žC'>?Â÷ÜgkìZ?·w ²í?çIáL$Š"?ε'`Žƒ?À¢A2û*?Á3O&'f?Â69œr«³?Ãü眱Ñõ?éŸàÑÍ£É?¬Àâ9Ľw?º­U{§?£d'~$ñ?¸þL?¡øÈvxmª?܉ReIþ?³ØLˆžér?ɜîêA'?µÙJ™L?Ö§ù7}´{?´«CÀ«©?ít¸@ñ?«*Œ¿˜;3?žF5oҎ?™hÖg?©"Ùð"‰}?¢ö{ùžÞ?ì‡qÍ«M?Áh3e]&ø?«zÕ.&KG?² Gª˜ØD?¬¹J'é?µìQªö?턑«þ9ñ?¦>ÍÙÝ?¦RÈzb&?•š'ŠX=l?¡d)IÍ?Œ= bU?ç߆d?¦çW—µv–?Áü£ÌoÒ? Gù­šFW?¸‡Kõ] ?¡Fg""AGN3FGL J2015.6+3709@R·_ßÏ?òø
€CRÀ7Ïng¼¨À:+l¤nò?ÿµðÓ×@rõJð>@@îݘͿáÞ³&¿åÂóýé$q¿çxýP/¿è¤ï‰ÌXDAGNFSRQ?։#0AøY?Ï{ÚW?"•BX%l1?•å×a…"ï?äÄTÙ B?ϧ¦BÊø?àk$ö"?׆"8_ ?¢8ÃèaN?£üRK|U?ÜáÑ~ÞS?ÖW5ô?âäéJå_?µÕ؆ι?¹w\¡ÏD¸?¦ÙÀ®?ö?ÓÚ-]Ô?µ¢¬êÇC?ëw…ü‹	?µá›KÄ{O?ˆêõ&¿#Å?²ì¦ÜÎ"?À":uØÛ_?µ‰À³Žã2?㵪£F‹?ÏÂ>ž¡@W?"À'¿?ˆNHÙ?×îª7î?Ï£–l,g×?蕐½taž?Ó!ǜG…?@rwEû›?¢{æF™¸?Ê®º×ƕ?Ñ$î¥YÁ?ä¶Ý©¶>¸?¶9ñ"ñÕ?»ÙÎõ¾U?¦X7§
6?Ï7¡àmœ?³`šR.ԇ?í°´I·ó¼?¡Â‹o#=6?»Ñ¡"?‰_
ÓÈ;?¬—6ù~>? Ď3
ÏMIXED3FGL J2016.4-0905@A+©Ÿ¡—À6úã Ì(bÀ8ࢻž§À;Bqÿ÷œ"¿Û}ˆ¯šœ@šÍ¥å­C?ÿÀìÿÈ!¿Ý(§¶_D¿ßÙ.ÁÌk¿àFbuž›?¿Ûj?ZD*cAGNbll?ïù¦é£??C–)ò|o~?Ѻù{î?ª5EÙ#Ê?Ej$Üïµ?B$Kþð$}?ïmE°/Õ}?'FGj«M?oש6±?|ñÐáK›?Œ¸©š¼±?¨É›¨t?ïLýïý?‡_JjÒÒ?†GIŽÁÒ?wtm?'òØ8á~þ?™ëÆY‡?	o.?'¶Nüµ?IË$úÙT?GÇãn*±?¦-ÁŒÛMÍ?'cÂÆYXE?ïýŠÝi'6?)xb…'.?ÞFxý?ïIógKÞ?.B<0=j?$ÉNnXÏì?ïÒäû¯?sw$¤¥?WJp|—è®?R…1GíŸÁ?q)qi'ú"?pvRõÌǃ??ì+?på3ù'4Ä?uÅþ8$?hƒÖÞyk?|•›t›v~?d'v¾>S?aL™?quËwüÖ?2ÞêÒh?Q?&Ú#3ªéã?‡1êc?pí(åäå4AGN3FGL J2017.3+0602@HOt cLÖÀ0:?–îÄÀ8"úgðÀ;×@Än@ƒ–ÿ‹eú@
S
ã2ê¹?ö'ª%Øם¿Æ‰Wu:rJ¿Ê£ö¿º¿Ü÷ßFïJ¿ìÁÄÜq
<PSRPSR?Y-=F¥µk?hÍéé!q?ï#ýòÎX?«§#'Ét?™ím×	€?«·4×oŠ?€¯¶\!ï?²'Œ¿Üób?íO#ú?»UqÃß	Þ?³qP½AEn?´VžÊu?ª'Á
lsG?'ÏƔ]÷?ë@îÃÓ»?ªÀ¯B"Q6?ºD˜áN?¨GÒ5ôB?Ì§á½>?|[r±"2`?íÞ
ñý€@? Ð6Ü•y?­¬s±Õ/?žZíÚ¨F?GmKä!xÔ?R'ls£•6?<:?´óí€<–?£ù·Wby?´ßR®?sšoúY8?€èìG!`Ó?íOä¦!+8?³S'%‰
?´G3Ϟ
?²¿~XÛ?«RƒÂƒ!ý?žé½)ˆèÜ?ë÷iG["?¬Ö²ƒVŸ?¹Õ_|ï?§!$SK ?‹SÈD ð…?uÓk}¡žO?î]ù|G'?"R÷Çº?£Kv*f¡n?Z|^PSR3FGL J2017.6-4110@vz4¿ÍhÀ@À?öÀ:få2õÒÀ;ÉdÞב¿å	 Å>ÛT@
Lº–@FônJ6¿ÛýxU¿ìæRµöп´U¶ÀÆÚ¿Ïš¼ÀvAGNbcu?ïÏa£Í¾Ô?u,_SR…"?"U}{h^?"ceÙCâ?w¼'³4d?tð…Hß®Û?ï‹b(‹†Ô?O€·C¥Q?kO¤=h?€/bYá{?†S­æ¨w?'ïúS4²?î5Êf.÷Ô?'|>D'Z?#`6´?wt¾²œŽ°?¥\U؃ø
?<™[5‰?ï_ Ès2
?ˆ6[G(§w? '™)$Š?#¾…3Æ?"ñÆ`´ç!?ˆ,a¬ý«?ïê0F³‡p?lž ò¯Ü?'>häÒQ?ؓIY–ß?e'/y?lUu8–™?ïڙi¦•^?i^"TE/•?R½SyT\?PÄ°מ?lì¨sGê?dù.òµ?ï>\¬Ðw?{³"TÃ?}±¥´¨?dâòùM»?È'aóÙå?x0
)'\?ïäXÐâÂ>?[x(~!	º?Þ[Õ
@J?-Õa1·?jø<'……?[ár"øAGN3FGL J2017.6-1616@;F'À9@"À:7{ßto>À9J
'/ï²À;rÁ3;–¯?ðºÌ1qg @Çö‰^¸ó@ц B« ¿ÊnЖ
¦¿áÔÇq\þM¿×'r%-ÙO¿î.
)y¡PSRpsr?âøó?Éõvºš:?Ò³¤âøÞ#?Ç5Ï£IyN?"QÖ-ëî?ÁŒ8™4Ö?Õ÷¦}éÌ?ÇQßrä"?Ú7ðOfx8?ÈñÁxÛ´?Ï¢z|?¾®çæAN?ßÞ¥Ýtº½?¶–Œ_NŽ?ØbûaN"P?´î\¢¬ã"?¾ù{	>JÇ?¤¯+qëp?ß5Ûa†®?·ðá"2âÓ?Î\CDDÊØ?»S–ÄÁÕ<?ќIi3(?²¬ÏxXX?ä85҆y?ÈBTä2ïì?Я¹-‰?ÅpÍ'eŸ—?»mÊ¡
?¹¿Â¶
?à"碪Ô?ÇÖ
ç¹/?Õ À4?Äؗ.7ÿS?ÅRD4Q/6?´±ò±÷?åvœÊ¯å?±ÌwðÚü™?Б9š;¼?°1ú™§?²ØðVe?›‰Àg÷{›?æs7&ª?«[³S*Ô¨?Ê	šþž
?©d×'1ž?»lFi	Ț?œØ÷&5ËMIXED3FGL J2018.5+3851@S%öà1-Ÿ?úžÂÊ £À8­°"—©ÕÀ:'õ}Åþ?éfÛ+_T@â»Z^›A@Ô6€šš ?ï·¸ˆ¿æø…cF¿ç{g;§¿×}–³é°AGNbcu?ٞúd¾?ÐnäH•?½˜çíå?¼4Páç2¡?ßöß´ŸÉ?ѯ1¹éù·?ÄS©†‡Õ2?Ë3±¹²$?¶Ù¸îs'?²>Ÿw$ß?è*:g@<A?Ë(öÌÙ·?×Ó,tŸ†?»$L·#ÿJ?¿"¤ù&Ђ?§]ÿYyßc?à2&‹b¨?»ùñwjßa?Õ
…ÌÕ}˜?»Š«·uÄö?¯ö.ÇFY?®Òù¼¸æ8?ã{U¨ÌÏ?¾éÐÇ5ç¡?áÍUýÒB?Ò*ôggå?°cNt{S¾?µ`d²-Ðx?ØL€f—¹›?ÑÚ4Lj?Óm‰ÜÉUZ?ÒU²W3K:?¸%[š°Â?²>¤?ãDže}«?Ñˋˆx£Å?åuü~k?ê?¸Š…Ó´¶?´˜4`ºû?¡?J'ý†?ÏÛóÕ¾ý›?¶eAÕ
ԇ?áêT·?·bÇVˆ{N?ªÈtPô_?šš<ÙYŠü?Ú³¨ìüJÇ?¸Tƒ BMIXED3FGL J2021.1+3651@RÎè_ÐJ0?¼éóŸÛŽBÀ5hÀwSôtÀ9Þè¬&d@ŒN¸@ý{|@ÛnÚ~;D¿ÕT.wÙø§¿á"~ièQ
¿æ¤7HÛTê¿íCÜq8/$PSRPSR?@Im¶òø?ˆØ™Ózè?ïhâ6bßì?™PJ³<	?'ÙiÀŽ?™ý0º)~?[Ñ7åÿ_?šxe{á¡?툦)[?±ÄT'
J?·w¤·í§?°þÎùô´?vð•<ßM?s9kªŸ°?ìë¼(\7?£ù³LØ|­?·Aﳈd?£$ß_*ñ?/ª›mŸP?C×ñîЎ?ïI¶?A´U?'k‰Jré!?–·lŽ?'aKLïÛ>ìÚßÈ,E>õ¹Ê×½WA?ïwÖ­:$-?£Â2bOkÓ?'ŽöR'.?£ÁÏÅã?Uv«OÏ1?{MƬ'2ð?ìhv›Š,?­@#:³?¼fpwa`m?­/[CÐ?vˆG_V¦ý?~¿šâØ?í!.åà]è?£÷—úµ?µŽY
ßÓ?¢OwCzËp?]ÐÁcÊ«?*ê§_2?ï8ö}d¦?AҒœjÓ?˜Ê҇Ýë"?7.·ÄÏPSR3FGL J2021.5+4026@SŽÔ2Tç@ªJ_ʕæÀ4Øï;Œž	À9҇'§
ö@K§ÍäÏÎ@>=@§:@¨[—ÖK¿Ók›
På:¿â*›Ö¤¿ç­»I–¾¿î9ïxPý&PSRPSR?¬cÞáG9?´ªEâƒ'?ë¿AÏ-OD?ÃM£Y?³þ¿–¶îÈ?¼RAf|·?tɬڲŸ??­ç!ÿ݄ü?ëÇß&¸óÉ?¿›-v
€û?À:5þ6Á?»R²ïí?À¤ÁØtm2?±Ä'¼Û»?ݔјägô?¹ÚQ«Õl•?ÚÍzáas?½ac¥Ê]?GjŽÆ4°?N_õ."N+?î«*—$Â?¦	`k™ŽÙ?¤ñCN8\?¥Áûǟ?¼D^X×?Á[JÜû¡ª?éS^SiÖÖ?Ǥ\¥6I­?¹ ¯S—Ã?À¡x©<­c?i_u "?'6Mnó¨¯?ì@©#¶z?¼Cl™äÌ?¾E?¾ö-?¹¦4¶Ú¶ß?ÄӁ]L?°ÂGýÌrU?àê¨òŽ?µâ9UZ?ÕÒB4$l=?·2km-Í?FDJ@ŒÃ?B—÷L>Ý?ïû?©‹?•å-ø¨÷?œ.uÇž?•œ"'Δ»PSR3FGL J2021.9+0630@HÐu@ýAÀ0ÅM¿¦sÀ9ªwhiÏÀ;m
[£"Å¿û»T­~«@
5#·j:@s\ <`ƒ¿àJ"+y3¿à`™. 
¿á‰ûcZ¿èø°1ze;AGNbll?îÌuS`œš?™©)x'a?†@ßÎo)Ó?‡U2®½"?›På±ÜAÆ?"áLê?îýHq.?¥'ùz&?°	#"x°?ƒßØé+?˜jï(‹?¢¬?çá "?ìÅu¿}b? Ë°$»?¤>?QŠÈW?"kŒó?¯oÙR}a'?–:bÇà?í\˜-#ú?¦n°N÷:Þ?cP̔wT£?k£i2'ß?´€¸4—êË?¦Tÿ£É$J?(õ0ˆ?"H"K²•?i®ÏqNð&?yû5à'?€îì7wñ?yÅ·è?ï³)ÌñÏ?‡Ãnþ['S?d9ÇV«/?q¼IÐ	>?|aü‰OâÓ?'¥nÁE?îúPUØϏ?ˆ¥W÷?ŒÐîÿÙgÛ?€¿µàëžd?'M}¿Ñð+?yÂȺ‹?ïEóàj—?ˆöDñ‰?7 Þ*àE??;þ§3{=	?–ãsu÷?‡ñŠp²ÜAGN3FGL J2022.2+3840@S6¸!ï?îÍÁ¿Ü&À7û_)[CÀ:G$ãW²@Óï` ~»@
e•ÙE¬@xH-Á.^¿ÝÐdÜÎw¿è‰œ*Œñ¿ë.P«>¡¿ïÿ†ÈÜ}DOTHERspp
?`|ºËvk+?cv‡eÎ\¸?Þ+ü~|mö?Òeôîvb)?àم\	?Ò_Œâ÷M?L‰ZÀ	Ïì?}éádBL'?êBüt/QÒ?¸(`¸7Ѝ?ÆׄÔĪ?¸!omIz5?°¡±j®? vo¯ ¥£?áŸ9eɪÑ?¹a™`\ó?ؙ Ù¥‰x?º<¾)úWþ?mIàÏÞ,?f)¢Í2?ô?êeÝnIy?³Í™ucW´?ÅIAÛfn?³œy³JDÈ?Mèªüpn?R)AC?Ý"ÿŃ¾w?ÑúM¬ŽÇa?ágæ»?ÑúeòM9ð?\É9ˆ"U?qNNd¸vŠ?ê~C:ÎnI?°9J°o?ÅÍ`¡ç'?°7†Ւ ?¸ýº«Ðy?¦Ý'uh?âg.êw?µs`ã{­?Ôò5-¤Ó?¶!Qùö:?s¾ì~á¹ñ?iÎ5XUšO?ëÍ3çýÅ?¦9äÅ_h?À-«Ìnz~?¥õà(Š'ßMIXED3FGL J2022.2-4515@v.F_•'ÍÀA:2 f<uÀ9°Ö?<VÀ;»>©ˆúæ?Õjˆ6<I@˜þi'@ÄAÿÿª¿áq—->㧿åõ7¿ßÔf¿æ‹"\!¿¿å³N÷^òAGNbll?ï§Xš¼ý?‰³Kð??r'é)	pº?xεÛȬ?yÁè$û?"t ™?îÁ݊V§ú?¤Ë ±H´e?'!;®;Æ	?‰Å¹¯¤øç?ž³°åô7¶? æ'¥"^?íBî>âhë?£ts°«øÐ?–N¢Xº?ƒÆƒÀ'úh?°Tår
£'?¡ñ͍<,?ìJžYqáD?¥Ú>ßÀ™?—骖%¢¥?‹oE<ˆ"?·°¢Žy™¹?£€_'Ú	V?ï1Î:jü?Àá4˜Žß?w;0†qOú?¡OCµ?"÷l›z=‹?¼Z#PÖÌ?ï™h/OŠ?‹Xò1À?lüùÓO¤¬?ri¦/ß?'fµ¿0¬A?†Oœ^mL?ï •ÐûõH?‰´ê'ajI?'hú¥Ûà?s&c¤¼£º?'¸È‡8†?†Ú'í‰Ùÿ?ï"zµl£?…°€þҊO?Ñ6æz
?g;Ü"M@?"9B÷{?'ÃõS&AGN3FGL J2022.5+7612@[Sc€ß@5#ô™=SÀ8߃'gMÀ;€Å¤º_¿¸AÅ(£@Ëbôkø!@ÍÄÀcÝË¿æ|V'0¿äs ¾¦ïC¿äYž¿ʵ¿æX
6n|AGNbll?ïàÿ†ØË?fº"Û1Q?]Nüwåg?Y':íìâ?`Xû@
ê?_[¹»(YÃ?ï†DµD?¥ØB»?‹Xq'0È	?±‡èe[Y?'âþ³ót?¡l5–çlô?î̚¼žL?'™¶^?ŠÀŽfd×Ô?€¸N#ó#÷?™aA¡P–?ŒÒKY<L?íÎáòEO?¤1óY]Ò4?'ÍÃL-p ?Š³ægv³?²Îbyb?¢eòP©Œ?ï÷V™ª?FgþuævY?CqcQ>?<æ%Ö*ó?>luñ "?8÷£ ôk?ï¦ïnÀ?§gº-˱?s¸0eŸ«?s™U*A°™?y=yI£P<?‡oO´—N?Ùø·ë?zÏÍ«ï…}?vzbC¯hÌ?p*´Â;¨?~¶°ÕB5³?rE<{??ïU°4ªpp?+áúS…?qB¹6bªª?`øK9:"?ùK ˆãH?€]·vD¾AGN3FGL J2023.2+3154@QÙÜßÔçNÀ']ßYAeÀ9nwºKÀÉÀ;6jö ?ëÐ^_0çÿ@ çiõ@'x z´Q?ížf5F¼[¿ ;'Z鎿ãZsæŠA¿áIÑJ¾rËAGNbcu?ï‹RÀ'‰?†rœlO|?u7Ÿt"u?rjзG¿?'€4œ€†?×ð£cÃ?Üç™ahÃ?ÔzçicÏ?µÚ>ç?°:¢`±~?ÝÓ 'VŸä?Ò¯}Ъ×?ìt³ä§°?¤BEq!÷?£E£ƒjg¯?" ä?êi?²·8'?¡å,1d¼?æ*ŸµVRa?¶6JÍî/Õ?¹éáÛ|½ì?°6_ jm?Ê`<èW‡?´¬Õ±Æã´?ïÌãE_/»?oә
£«?gÅL¼‰?cÁFßÑÏ?kW³K +?b4 Ùu ?櫐EC<Q?ÑwÖ3[¶?¬ *┥¸?©]Gm_)?ÎI´1¨ø?ÎV ¦œ??øè×?•¶¤Œ®?'¹–γãº?…a2'°µD?šoG99`?'œþÀõ/?ëâ7œ´?¡¸<WUC­?¨®('ˆh?'h"®
?´ì‡2{â«?H3X¥'MIXED3FGL J2023.6-1139@@O¢ŸÒ˜¿À9®â_ܪÀ9'`uÖFÀ;T3—Ac?ò´bÞ©ª@µL¨z2?ÿV´öí?¦,EG ¿­¿ÚZ"|<ø•¿ÙÆ»®ÊáÄ¿çz8B'ŸûAGNfsrq?ïN˜‰½¾?•Ò·oòB?%Óç,ÑC?"c9‡yö?xkòʓß?r|«÷fÁ?ëÉivCܬ?¹f@a[*?ªI"Øg@É?§Sä·,Û?´ñ߇¸¼?´ƒ¦¥Ÿ ?ìÇ¥úÇ?¦Fÿh·kÀ?¬Ée–0.?ŸQ½'Œb¯?¦¼:ÌbLY?–Jîè€]?æìrlâŠ?®`ekJÃ÷?·ÂÀàÎ?¥S"è	&5?ȅÕJ't?ª‰ûÓÝ ?ïºâL™iQ?€*ínIàý?yHýáËï#?|š³~¬Î?b‹·ÐY¨Í?ZaƲú'?îòTñžé?¦PȒ§ù3?œsk£
][?•ÀÁD¼7?¡G$á°¼?ŸZÇ ßØ?îËCߗ™~?'²Â*I?—&jîx~?Šl¬<
ÁA?Žü»@͈?ÿÎ9°ç?ë\,Û͓?•ìcs i?´ÞUfÊöo?ÞÚÙ²?°@C»6d{?
á*ý©AGN3FGL J2024.4-0848@AƔÿÖåUÀ8££Àd¾À9¹Í°!›[À;[Ö¥"¢à¿Ð&m2ï|¶@—pÛà;?û=ßÿ¯x(?ìñÐÖi%¿Þßo1CD¿Ù^ß§¿È°ÂHB®AGNbcu?ïú?PšC°?@"÷	2?$Ap?^?" q#š˜?AòbŠÀÏ?;­wð´ob?ï|íßʉ?re ?o6Õ®Kñ?ýnPñ\?ˆö玫:<?‡ÂÂÊÏÎ]?ïLݖsŸ_?&WѤØ$?€-šNÀ?p4¾² 1?Œ;md=‰|?v€í+Œ(?yÈÃÔ?•H"2Ey;?<1¶44{?@}UP—§ß?¦mÔ÷lY?•:Q,ô?ïü'Ûç?0ø²8W¾?&	Á/u?Öç±3½£?77œÂÎf?*&ËCY&°?ïÓUÚ¤@?q©¦-,D?V5"XÙ!Ò?R™Š7¡`ô?pÈò(ÃÅ?n:qáÅ?ï¥zýŽP?m	ƒaíR?rý[A±?_qæ'3ò?zE&kGÎU?f8›š€?p?ï¬ÊÅäž?p
µ^"àu?-–ÖG'7y?!ÒmŽî3›?"VóX/Ÿ?oà—sfaƒAGN3FGL J2024.4-3254@#>óà¿À@n¦`QyoÀ9<ÚvÙ{1À;@#¾†À°×º'‹Ù@å5O?b@OêÀ'ÍÏ¿éÄ:ê.)¿çØ
Ù¤¿âÉ	7¥ø¿ï¢3äÔAGNfsrq?ï÷4&Î?L‰‰:ô™?9r[uùÐ?8œN ?Gԑ>R?FюæA<K?ï‰ùº&é	?‰y{üV¦?jiŸ*öÎ?|Ís«"U)?†çPÎÒö?ÉÁ(û‰?îrzÂz»?"ê¸R`ž?™;]µNA?‰>6n£?˜uIþݳR?‰t'¾6¼=?ïˆÎÊÜe?• ¼H|7â?2\ú l?Y'µêøz?M$mj)?•nÀ§û\,?ïøöfN=¦?DT‰bÍ$?<dðŠÿÅ?8f¾hZö¢?;çÞH‡êÑ?8M¥Y?ïÔiÓûŒ ?{®•ê	Œ?WLÃd²žÜ?máªÁhwY?oïÊ Ÿ°©?oŽ®Ì457?ïHUsá?†ïX#=Øå?Ž/n‡¼?|Œà7µ'X?‰'‹¸m_Î?ÎÜ?ïë™Rï2 ?nMtth>ãšE‰ú?hvô?dSª¤gS¥?nI'Y_AGN3FGL J2025.2+3340@RF–àU­ÀOÖOÀ7é£?4É5À:^zb?øÐ{ùF@…'Ԇª@ئ²†Ði¿â±Àç]¿¿éŠù‡"³¿æ"@¢Ã ¿íÍVœ2¿àAGNbcu?èüt'Äý?Âüúz…?°£*âÀ?±'+½•¢?þ1î(€ì?Ád¹cʐï?ão¹¡Kë?ÔgE׿?­Ö¾Á…ì ?³O"‡âÙ?ÕBH´úž?ÒÑL'9Å?âñО­C‰?¶ZÖºÊ1`?ĕ'k³z?¬Xç;ÑS?Ï£+jß>a?³uŒ"Me?éCæ	ðÕÒ?ºè^HG ?"Y‹¾©?"¿Sg†!?Ènü¦Èðä?¹cMj1›/?ì:B¿uÔÌ?»ID'ÞR?°"&Œ2ˆ%?±pIc•3€?«3†ñõpó?²äŠÿÆöÔ?ê;þD$X?Ì_AÀ%Ø? RáÕ&ö?¢ÙÈ–?ꉍÕ7¢?Èa«ÿÖB?äëá̍?³²}uC?ë×G,Âß?©ÙXOm?ËÔy1¢Âì?°ccMhyÍ?ìŠõZ›¾?¥Äi]Å?˜éñ!  ¸?‹ƒ`èp?µmØáp,j?£â:õ®Ê,AGN3FGL J2025.6-0736@Br® 9[kÀ8d:ঞeÀ7Wm¯0ÔÀ:æX"»@ܺ«@7ï<ä7@xãPÇÄ¿ßRáù§u¿å¥¨×¶F	¿æä¦É¿ëÁuuoe5AGNfsrq?ï¦*—?…YXs?u¼=•?€i~:±€?wåÚî®3?xNxww¾"?M˜T?‹È.š§ß?l#úÖ'mó?}Ô`7ޘ?…­Ü‹uƒ?Õ"í=BD?éE›ªËE?°—âÿüër?ÀÌÈtgIÕ?ª.D;7Fe?´9'+$ìª?£Óåô$ÐP?ïÚ>áxfª?€3'‹SÌÙ?7/mwòì?^ÙºF~¾?qo|-XÃÞ?RqƒzDQ?ïÂö"×Ï?±lB?môZ…´–¿?{`}SÊÑ?o ÂÓÐ?mÇÛü¢?ïÔÀviz?sŋü'LX?X^Õì纆?X!£¢‰½¼?ox© (¡?n}
äªÏû?éòcH5	2?¯{±Àª?À‹Ê°¤?©E+«šò?®­°LÅr¿? ¶ŠœúÂÁ?ïù€¶¦?[èÏþب?#×x8¢^_?3­†*çã?EJ°&À?ZòÀj~z
AGN3FGL J2026.3+7644@[z°<«'@54·¿õMõÀ:"TÊÀ;ÐóöÝA¿ò²cЦ÷@·…:<ý?ým8ÎAl?ì™Nw©§%¿½†"¯¿ÜÞj)К¿éäÁªÒ'AGNbcu?îÊóQ×õ0?¥%­êÂ(?—Ãq%ÔrU?¡ãæŠ\<?¼I-+Ãc?–?¯iûÌ^?îaUè¿Ç?³¬Ý™"Ñ;?˜á&…²é?¤9T7ú=?šôb…]?ª²Qb¨~ª?ëÊpO"ˆÌ?«$6\†´R?´VD›'°?§íq6Ä¥?ª¬qÓûìÕ?˜ÀBóÃÒ?ìætþ|Ä?¯³íÊ÷Ÿ.?™õdƒ}ǃ?¡ VÚ5µ?²Nþêdÿ?¨"pÛkh\?ﬗ/±ôY?Œ¸v×âOw?w‰^Î?…¹‰ø1—Œ?r¢Þ¹I½W?€k	("¾ÿ?ïŸW7Ž%Œ?•ùxÇÿíè?uŸ6z??€™Kzƒ¨?z´å™·î?Žú¿Ðð/ï?í <S ð?£#Ó'†Œ	?«(›s7? ÊíåÑI—?™»½=µ-¤?Ufi	'¡?ïUè¦nÖ?‰¸ÜØ@ù?dfˆ% ?eM±è¯Ä?'¶4²ÚË?ˆ°:¡ºÅüAGN3FGL J2028.3+3332@RW€dÀ	¾ÀD©'À7xrϏÀ:pŠ)º
­@VVù¶æ@}$îÌÑÕ?ü£_9M¿²²U/åÔc¿Ú³íéä¿çýuûÉ~¿î:öå¥PSRPSR?<ó`Ÿ=f??«0Å×4?ïÀ‡¥Xó?"x\™ô1e?}ì÷H!0?ƒÙ­ï³à?+Ÿ¨oQôÎ?FÇÛñƒ?ë@Ðlêd?µ…b0‡î]?ÂõÖaÝ%ò?µ|V‰@ßX?~ú#zõ?vr,¯–Ê?ìqe—xEü?¥3.`ӎå?º…1
lž?¤©Frƕ'?o›b?¼ã´?d·*ñ¿¤1?ìí¨>osÎ?¡óVÁ†1X?·•âüuB3?¡jM—0µ_?%ÍœŠ5?+7èV¬?ïàþíœ"?r>ô<<n?m¤¡|ÀY?qºÁA\Ko?S›—Ëæ)_?ƒÚþ2‡Q?ëP%»ëÿ?±Â	ò&‹v?˜1á4Éò?±Î<CR:5?‡ÌïW?…a(_ã¹?ìüô+ÃË?£ÅVr
ʪ?µÝôÑô`?¢ødsO¶?yNùC‰?f_Ω=>?ìÞÍ­óBØ?˜ÔÔMâ›r?·y=Ÿ?—Ü,Ä·³PSR3FGL J2029.4+4923@U˜WŸúë@Z
@JÈÑÀ8rÞN«_À:úō=jÅ?óÁz´&8@o*s*©@I:ÀETô¿â½'ö{-.¿àb|>Œ¿égóI8X6¿ì
GÃ^vAGNbll?íëhªt™?®ÜÇþ.˜?°™¼zhR¯?­‹&	e@?Š·AôaÔ@?‰ZH³¾'?ìå/ÀÉ ?¹šÇcx¬?"D€wÀž?š¬Øl'nj?³Å€+OX?µ1ðž%Sþ?çÚà•pXò?±Õ‹ò?Âl	²¹Ú?©˜È=æ9?¼PñAĺ?§|¹?|Q?ëôKۏw?©òÄ [ê1?­\Ü-u«"?¡'xÐ/à?¸qï‰úºþ?¤Æ¡:|ò}?îºÉðN‡"?¢ˆö…'y?¡ãI(ýu?¡«örËj?s€¾}'ö'?s•HN¿Ö?î´ÎÄÑ¢?ª"GÞÅ?"3Ãÿ"<3?ˆÊ'ú‡ßÍ?ŸLES!œ?¥ÝŒ›Uó?ê¼ 'F¿?©%;QNw?¹¿t_"zS?¢–î4ÂB?°_‡
]³%?ž#õûȱ?î,Z£(}f?'gÅS_7?šV5ú_m~?…›†ɹõ? :Ñ$YØ?‹$Ϙ.4œAGN3FGL J2030.0+3642@S~ +ïr¿öçÇ¿Ç«¦À7΋ýϤÀ:ž;aÕÝî@øByw:I@ړ‰à?ø»B¶³Ûº?³ðïèkõÙ¿Ø_ÄŠŠ¿å«Lh¨#å¿î"¨FNPSRPSR?$¡o	œò?&NµlÄ?ï»õý˾?‡€û'Q
É?€¯úþg:S?‡[®Ë†°ò>û£"·AŠ?åý6e?ê¡âþ½_Ç?ºƒ:ñS?Åw–éªÂÑ?ºƒÀ(úu'?'K¸´=¿?Œ>ُ§?ëê7æ:û?¦§Ÿ¡Þq?¼[R¡ƒâ?¥‰¼·ì»?V;ñ;϶w?S5+¥f'?îN•Þ½ÔÑ?›5•'ð~?ªd‰hN<?š³÷MZÏû?í"6>Í?¾ÑU÷?ïâÌ1,®ñ?ŒzN—ì?lÐz£¶Þ?Œwó8›?+&aÎøt¬?_^jÿˆLô?ꈙ.î2¬?±5n4?ÅÖѪÏn_?±ˆè<É?–›Ð¡/Êz?'¢Oöe"?ìdÉÒ,Ä??¤'?8"i?·2½G)Òe?¢ZW6)ä?c,ž\¦?VŸˆ3Ô7Œ?îEöû¼5?'TCJÃÍ¿?ªmÔùÿÑU?Éy­¬PIPSR3FGL J2030.2-0622@CUv?ø="À8Û[¿CwNÀ9C†åaïÀ;[?ep!?ÈýWlÈÎ@'5·œäÓ@ 6à'Т¿èOÂ)I"7¿éPH÷Y'¿âj˜2CýŽ¿äòŒ~ËY}AGNfsrq?ïþ#â2d¬?&ÍG«çM>ûs†æ)¾>öÿPB$Xÿ?*^/7ÆŠ?$×
Û³qÈ?ïŽîbu?"@{ÇÖÖ¬?nGÝ*è1ê?€Bu.	?ˆŠM,uØ3?úFÖɾ?ïúNÔé?"
ï
f…?ƒhe•q†?pC/{×à|?•lƒ£ók›?€ðn		Ì?"ÔR?~-´¢?2
dK<í?40À"JGï?‡‹ä+6…:?}Ìʋ6yï?ïÿ	‡ï?¿­Ú{Ÿï>ú©r˜õF>õZ.ߕg?%¸ß¥b$?]WÙjˆ?ïÖ{z}RD?m¡ÆI¢?UΗ~ì'?RC¤ÍÝ¡?n9²¹[B?gý=Ó±?ïž~¾!
l?j›6=)Ý?rΈ?YŠùïHæa?~½™þ—=Õ?dzÀ~1u?ïìôQ˜pq?UÃîgt¬?%җl±çä?ýbr-j¥?a®"ýF7€?UB˨ɱAGN3FGL J2030.8+4416@T–Z?çvœ@ößoçšÀ7«ö©?)À:|^ʐ²j@©'¿šÃ@ã$ð_?ûé/Ï%—"¿Ôd=eÕ፿â
ñ!bGÀ¿èa9çéo¿ï·},¦|+PSRPSR?a€¬K«Õ?eI3›?ìÓޞ}Ñ^?¿^êñûÛX?¸Õª÷«l?¿þ'íƒ?0sV ?DNjÌ|ÇÞ?ê÷Lu­ë?¸dÇ~ÿñZ?ÄÁM*ß?¸dk4þ?…d*1ŽÖ?€¶±nk#?ënFjÙ¤?°xs½`?Â8DC?¯xÝßµ*ñ?`-çÌYîµ?W†­n"`?íoÉÙþ8«?¢	d•œX?´Aò¨Nt?¡ÍÛmœ¢?XÞ±ÆH
µ?f€^ac?ì[,Na?äÝ$]ØM?¼Ã$yÔNÄ?ÃrŒ%WA?Sf8ÆP?gi¥ÁNZ?ëxf'~®?³
èõ/>?Á÷™GAæˆ?³ô¥f¨í?'sõ§(ÑÅ?‹±]ñÒߙ?ëÜÒÓC?¨"Ø°ø:?¼Â"w–‡?§‡úÇÈ0O?jô7O ?[Èoq"õ?íK'¥‰'?™Ìoö+A­?²E"ÈtM…?™7ÔÃìGtPSR3FGL J2031.0+1937@O( 2:À'`ÿX±À9¯˜JAÀ;o7…¨K?僧GŠ·@ÇJ	
šÈ?ý5ëˆ"¿ÛãÅñ«_¿©;!ØܔZ¿Øð8^¡`¿Ú·Ñ‰[D0AGNbcu?îs¾#Ë{?°(LA7‡ö?uwBWÅ7?y™éÏ»B?¦,dœhª?¯çÿ_Œ?íUîڜKÙ?´:úfˆ×?'°µËñ‰?"|&'m=?°¤[¸!>ö?°÷#êø¡?îQxpT%ò?"i8ôUab?"ú=0R§D?'nOª<s? ëZ_$±C?UîwÃ?íÎà‰~U?ŸÊ(¥-h?'‰?Ãà .?ŠLFãÉ?³O9áÆÌ?*.bû0?î݇¢h?«Æ,æ8ù?nÃhùRa®?uÙª$Z#? ;WyK‹é?ªI
z¡>¦?îк6`þâ?¯C˜¦¢?^Ê<,À?ˆÞG7eá ?9T¾íc?©órj%š?ïZ–/h¹?f¢åˆÏ?[|3Gw-?q¨G:åp?‡þ÷éÇ^˜?wƒ`?VgK?îçîe<´€?ƒd'(ù ?Šl¦€ä•6?qÅL¹¸¼(?•Ëà?We?­?|	kZAGN3FGL J2031.8+1223@LÈ bÀ/mÇÀ'áÀ9Kƒg(-FÀ;4ÎAAð?Ô¥}}a@§ÃþÇò@yF÷¶¿ãQßy¹Õ¿åŧ(Zà¿é\1'&ç(¿ÝôÌõUpåAGNbll?ïía9¶ì?ZÕ÷¢»»?Mëˆ'Ì?PéìïïŸ?V®ÿ—ÝOO?QŠ¢úÁ?îÿ'NºE?¦-#ÅD&Ò?z/…ù?z¶Ë—¥V?™ˆ[h7u-?£ÌªíBÒÒ?î±Nåsë=?>¥È ?2¤'%2?€vòz`?™£~ÂA0?†t÷Û
i?ì3¸­õ¶?¢ŒìûÕô ?8uv&ˆb?|Xóòå•
?¹ÏS‹~Š?¢#Á'Šur?ïöƒoê&X?F&ʐgB??â•^À?=bQ'9?F>˜Ï{W?;Á.ÓÕR?閭a®pÁ?ŠA¬ƒè=¨?fCÂI&"³?d¨3ûÜ
'?€ÍwÂ4‡?†pbHšr?§=#Õ?uÂJ5UéÁ?y˜bäÞè?l¤C+!ç?dɞ¾?mqÍ?àí?ïxz:±?ƒvŒo«±º?nu¨è²×'?[ʜÜp4?›B;£jú?'~V~†'«AGN3FGL J2032.2+4126@T
ýòÿf?ðMô·ÍÀ6'•¿†À:ª¡(Ú@ðzú;J@
*÷%æÄp?ü†!'Kòr¿¿KŸ:ÃJm¿Ù¢#ÏN¿âmA'3ÿê¿ìY!d(ÉxPSRPSR?"ÞÙó?sžºk"?îj.MyN?¯vh~Möž?©K ›úõ?¯r}KàG6?8×eÓ?ra $s?ëþØ~V?°tÝnè†?¿ðd¬|ö ?°<ƒd?zìZ÷¿_?z˜Yþ?ëÁHêÔí?¬[¢PíñD?À#|Å+ s?«à«º*:?I&_£?I.$?í+ºo–Õ‰?¤ù¾p´56?¶oî76?¤Þ—ª 	ó?@1­Úêú?
<4€Š‰¦?î'ô+?©Óbµk'?¦Ú/aǏ.?©ÑŒá5 ²?G×K'IgŽ?dœÊsÿž?ìõ>8¨q?ªðÜMR¬?¿H§tß·?«Þw"î?»"Çð°?'­cÔOræ?ë ·T.oC?¬ÝÌIPHE?ÀF‰Hµô?«ú—þgc6?Nb˜§ß^?D‡|ÝÇ
²?í)'³ð?›õ;tØì?¶{–èw>?›Þ蒬é£PSR3FGL J2033.6+6309@XŠ?ÿÊP@*þJ`vb]À:k£¢1ÐÀ;Ä×09¿"Þ#õ‰¢@C@1"J?þRa~Ë-¿êÌÀl¹‰¿æ"Û|	ˆ6?–Š-júÓ¿ÖŸjO:aAGNbcu?ïM'Ö˜
å?¼#iÞãG/?C¶i·f?Q§Jó~?•´§}bh?¼Ӓ
ß?îî},Fº?§ÔüÛ®'?|?…ž\nb?Žé†	ýa?› y$&(?¡ö§#¶a¨?î‡//~®î?"iyíâ0?†Èk•Ú…8?sÖ
Êæ'?¡Úò 
ºÙ?'Øß±4+?îðàÙ&Õà?"ÄâS¹éÛ?Us3zï6?e/†ýËøZ? FXÓ ÿ?"Oߘ)͜?í÷3¾.¶?͚S†mu'?k›fÏ~|?špçuyè?®Ìvc$5Á?ÌPG{?ï½Ð"Ë9­?'\P¦G:D?a_e™ùm?^NP;Êåü?xh;¶	í?€E˜¾çØ?ïR­!"Wï?"[Œž†c?yÁf]ž>	?b£odö|"?ŽtsR:?'Îom'Û®?ïÅl"èã.?h¯Øƒbî0?Q"{‰?GŠ–ãé?xè϶Xæz?fÿ¡"ÐAGN3FGL J2034.3+1155@L?› 'À0|rŸYÌûÀ9±vfŽªRÀ;wœÏÛ?åŽJݍ©@ÅÆ"8@̵ `]8¿åq¸ÆýÍB¿èÍò¢Ûré¿æ÷£"Šú¿å†>•^mìAGNfsrq?ïÛã¸nz?{ÝÝÊÚ±ø?WÖæöSŒÐ?cä¼MÁE?h0ÔE~o¶?wc"׌?îÇzBïÇV?¨¾ŽÜÌò?'?¹¿?‡°''¼#á?ñ-?®_²?¥ÒrbîÄ?îU[œ¨?–t›QboÍ?•òd‹A}?"üv³'?Ÿkl=H"u?‹ÿšé•?꼸ÇK?²ƒ—âèˏ?'T­÷≩?‹.,.Uì?żûNüx?±¨e<lXH?î²1öºi?Ä´ÑÙQ›?}–p¥E¨?£ß¬ Íä|?¡*‰UºÙ?•B$›Hy?Ž¨W€?€ÕÇ?kèUŠe:?l.ð©nû?"$†î]z?Š‹ò‹$?ïa34›ú-?JO»q^&?ž2)îh?yBÒ'̘
?†Ãx;?u«"¬†ë?íÓnw,n?•"{0j.‡?Œûè•Áwù?yz()²³s?«Šfm!?"·öoì¶AGN3FGL J2035.3+1055@K°‹ßœ³*À1;`c'À8ihÎör¹À;'ÃbÀ¿x?óÉ®	h4@¼0V½@¾4à1ƒ†¿á'Zr^¹–¿æ†?"ë_	¿æ´KÀÈ¿êAë1^>FAGNfsrq?ïñs ø·Ñ?S@Ô]ô'´?PRø°œüE?JdOÄgÁ?IŠû"?C*³:àÈ?ï$–æ¿p?™F$i¦=À?{¾|w~Í?|†Þlaœ
?"œ=ÎsV?–*
WïA?îˆh¥
ž­?"o1Ô?˜Sìÿ+ˉ?Šñ?Dyܯ?–žþ`Ø,Þ?†ÿ¯œ<˜?=3Öá?™àºôæ¥?yãF™"û¥?vêÁÃ?¢³\ÿ®x?˜ÿ³Šùœ"?ï÷Æh¸-â?Bùa^Ivh?Dݾxq¤?:´"^ùÛ%?8?n.µ?1Ké¤'?ï°ö4¥#;?"Ô‹!¤?fC-ms»W?aÍ=˜aj9?|cNí'n?}UFƃ?ï+wÚa"?"É)•'×?Še€)´?ìâ*§Õd?†²V)?uO àÓx?ï£}6Æ?yø`""|à?mãáÖ
,'?_'™B£=?O…e»^Ñ?wïI7x0AGN3FGL J2036.4+6551@Y(¯ ê[S@-ÒA³ÿÀ9¶ñµºaÀ;¦‡dã¯?âG»){_@¯^ìI"É@€-?¿áDˆ¢V=¿à¢8±ø50¿Ó¦ã¬ë¹€¿å‰_ț|AGNbll?ïé1ê³½‡?bèjÍRRŽ?X¥"6žÆ¬?V}­~E?Tö–·zu?U¡A"]àï?î\q™åÆ?¬Õå‡%E+?'Idêg?•™
ÖÝAÆ?¡"[07?§>7—Gº?ï2¼¦ö
?…¨]¼$²2?…&¡£€«?u<•ƒÄ?'æW"9Óù?~»l~‹§»?í°ç®Ðb"?ž4в®•?'s¯±%Tã?ŠÜ%qSÕ?«·­:g-V?™H¨\ÍWÙ?ïùhËÕú?CO§ø©¿Ÿ?8ÒbÉùJ(?;a'iöëß?;çFÙó0:?7}‹#Ï@?ïs"ýg87?';ŠUêÿN?x›Nü¨q?qÀ;GEŠ?†ÍYÖ?:Ý^…ëi?ï™OÎ/´Š?r@-íy¿?wœí ~J?l(_E]?|G{õ…ÜÛ?aµ_Ñtˆ?ï;¯(Þ?€;^Ùå¬?ˆždb2Ø£?pIßW#?ˆqë#·Ü?w&4½aøÖAGN3FGL J2036.6-3325@#X+€~
ÀA½â:¸cÀ:žƒujæ(À;£Ýs
=Ö?æז(î-<@
–B	òa?ôàÓËr/?íš|˜ì¿ïïrȖÕ?ï¸t´™
?×K;IÕAGNbcu?ïhv$Z¹p?˜1öCÔñ(?0_×Q‰›Ÿ?4x¡Å…Æ?'¯¼¦w§?˜"
­"ôˆ?ïm"¡Q?Š'-V´Ét?gÆQ¤À?|‡y.ˆµ6?†³¤NØ?nþsŒŒd?í‰óÍ}Ýã?œ?¿øAß?™Û±—T?"…ØüÃÑ?ªrêZÂÓ?–·µƒÍ?î*û¹ŸH…?´Y|¥ÆbJ?;_åñ·ÝR?a­k¡¤V?­"–•<Ä?´RÇËv¯‹?ïŽéŽß?"4£ÍYw†?6ŸS+.?Arv"¯Ä?‹ÀºÂI–?"ÿ;ïKP?ïÚ'>eôÚ?jñ	VÌ?R£:Š
ã?O¾5P'É?l‡${z>É?eÀnJƒ'f?íä*øYÌ? Ìavì?+ß*=-l?–y)Uœ'1?£'`æüw*?—jµäiQ?ï±Ñ«½•?Ï‹'—ÇÓ?;Þâ°\u?Sø±=!?'¬¥ABír?ge›¹z"AGN3FGL J2036.8-2830@/Êœ£9ÀA2¶­À9·'%VўÀ;ªÀ:ñiš`>F@í-–¼¡@ž˜›ü ¿â´låö-]¿å¥F‰Yä¿çÞùÎ@G÷¿çe±jFAGNfsrq?ïîBúE?Y¸>ÆÊ_K?CØ.ˆ'qK?AÐBæY(?YÝd;=>·?V xµ»9°?ïscT|ô?Œ¸FnSŽ«?k‹¢"8Àå?k.8¶?ŒYþ˜¾è?ˆ®–¦¬ü?îÙ­ .*­?ˆWØ'J§?‰%XRr*Ï?v·ä…•ž•?˜7ŸÙ˜šé?'	¬©å?îôW]_Á?"š
 ¾«;?V"ÛÜ߃?Wªùh	G]? cT4Ëê?"2+_úón?ï÷{ây‡U?IÞxY1I?3[=AbñÁ?2J'îºö?HbÖkÏÒÄ?E+-)Rº…?ïТÇb!*?q}5sËòç?V²¯"1?QÇ£
ÿі?rð¥W"?mºð\A?ïŽ~P›"?rÕP'»
?v¼e53Êz?`DZBVÀ?9Lœº?jWNš¹?ïȈ†æ?m:O¥m?)âl9/)/?$aÿ¸Òö?zìãÃáM,?m/¿Ž]iÕAGN3FGL J2038.8+5113@V/×,uª@Ò½ßôò±À8˜ÈQ=	vÀ:¯ÚM¾Ð¿ü"ƒèØF@ŠÆóïÑ_@!ÙŒÂÇ¿è~3•6f!¿êö°Šï);¿èó"ëxš­¿ç·Õˆ¡éAGNfsrq?H¨¡†?›ÊÆÑúÍÖ?@ÓH–>q?A˜ƒN1¿?Œ9;¦mi?›²$Q"\:?î7@_W?¶ÂÁ):¹?x܇¿	?†Û÷m?©r«
øJ±?µn›ŽX­?é÷*‡ą?²ÛÀ¿'†?©#"
Ki¡?Ÿù	_²ë?ÁÚpày
C?®Y TO¶Â?îm\"H?Ÿø*m–w?2hÜÔ[Þ?8ÝËÉ¢*?©4㼜a?ŸêÜGãK?ïÍ3Ç؜9?‹4úþ?0aæà¿ò}?/ÿ–ÙÁžÃ?x_ýª†ïý?‹Z@|ío?ïŒÿ8@?¢Ïí {â?d8ü%uõ?x§´fÝÛA?‡¾#¾Uxž?˜t4eï:?ízíŠÃ¤?£€;"I±K?•i…±œÄ?Œú=C8)?­œdq'	J? é¹>:þM?ï‰i§¨>è?}¨Œe¦ek?yxaî?#ŒÁs³ˆt?‰òbà?}¥_)ïPAGN3FGL J2039.0-1047@A£Rÿ" À<½ÜŸ¨§TÀ8¼äÏøÑ8À;8E­‰:§?÷8(Øîn@£$¨«Û;?ù§´³Pz?§†õŸv¿à:3Ïݛ¿â}zvÒ¿â7è6;6AGNbll?ïê?cӗGÖí†?FÁùß-@?D¦˜øþ«?`Z±q½Š¢?`È©*Éë¼?îe-kÈûÝ?®làH¡?Œï¼b‡¹¼?•å»v²:°?¢q:-bÀ?©øÝKÀ?ëØ¢%"Hú?«ö[ë§ó?­U`Ï`–g? %³T
{?²>l-lù?£ädö¨'!?éÜè•Í~›?¯ÿ¬Òi@w?¢Ò֚3¥ý?™yšôÙ?Ãר*;W?®õQW3ä ?ïû2=p™?7p/`§Z?/w-&o;?'OÖ¾ºÑ?6²'(3]?/è\‡M'?ïl¼³Çd¥?–QÎ'5'?uÔ×7%Ýh?{CÉR?‰æghôÿÿ?'i°_é%œ?í߀$
â}?Ÿèbžh‡ê?¢~FÒ®Ul?–WŠÆçi?Ÿm×/7Œ?"1dvÙŒ?ힹ奜î?™®Ä¼£?ž®Œéߌ€?Šr^{½8ü?¦½-FÎà?'þ(›qä^AGN3FGL J2039.5+5217@VkΠ£¢@
æO†%À:'r—ÍÀ;_®FÏÈ*À7Õñ
ÉÂ@
Z×h\4ß?þGàðñ?ÜMâ'QåŒ?ëHo«¿âP¸S¿Õ¦Ð†73•AGNbll?Ѐ‹?Š+ÉÁÜW$?Xoq#B1?TÞìIÀÄ{?‡KÁ¤((?‰ù—âÞ?îHìO'?¼bfD¶
?u²"(ÜÛ?"Ÿ'û÷yø?¨ºüìc›?¼x|é_«?í|å}ë	Æ?žªi '–ô?–Êî@Þï?ƒùˆZj¤K?¬Ì0ýpP?™»/µ]?ïnKHd?"êî¾²«?;n¥ƒ4±
?RÌH»0!?Hø'#M?"Äíàa·Ó?ïÓè\Ë2?–ŒÈ®b²?B¾ÂºüS?G
:hï>r?s³ù?')G?•çŒU^7`?ï¢Gî"ª?7A 5ô?_½Þ4­&?a¡»{¿‡¡?ƒ"2@¥OÆ?Œ9}þr1,?ïÜÎÖ?ŠGPcª%V?‡P#—å?xÛ°4y¥ý?"œTž«A?"—t–Îå¶?ïኰ·\<?l'H±>èCP&Á–->ýÿé½?n]ÿ©¢2?kþŒB…AGN3FGL J2040.0-5734@u:jŸ{ZêÀB‡ŽèӔÀ:O»¢çÀ;¹Åԋ0¿þî5'³÷>@
ú…\ '@'Ñ`w‰?휃OÄþ¿éó£ËC,G¿Ö[âé2¢Ù¿ìK%99KjAGNbcu?ï™ ¬Œª7?‡â°rÃ?p|¿€Í]?vkY™7V?µ–ƒœMš?'bæþ"?ïk9È+[?Ñ¶–ˆÌ?lݱÆä?nó	§ê"_?úMÀPˆF?‹|þfƒS?ëœÑ'0?£Ô;«!¸T?²çEE,І?œô;|lˆ?°2.4Š?—üqÏ&ù|?îm§™KŸ?£UzÝú_?G º"På?[©ÓQW1?¨Ç?>ÓQ?£3àŠ,?ï»}Êä×?~Õ%»@Ri?i#ø¶í2å?oö"wòü÷?u¯(›'á?tæÍ-Šœ»?ïÒ	ÑêÞ?q"Ô^¨9?V3«e`bY?Sí+&ËL?qn'F¡tŽ?m8'£îè?í8kâ"͍?žœmŸÅ̋?®8Òw6G?šQtϦ??œ€Þ» wÑ?Œ?E­a·%?者$ø)i?} "S'?]âçƒ}y?$æ=)ŠÌ¥?…ºìOžú?|ܞ,K»AGN3FGL J2040.2-7115@t2gŸì™òÀAá`xÀ9§™hò1áÀ;†‰1l‰–¿×ñÆ<Ÿ@
Õc¥ì¹&?üÃöM½ù¿æÔcGß"÷¿ÕŸ–äL_¿Ö˜÷f7±¿ÑèP©ï/×AGNbcu?ï›ýî,ï?‰…nÓZK?Sf¨iŒÔÄ?Rƾ±ÿ0•?†Í«~zW«?ˆ'E6­ö?ïvéùX¾?Œ©'ðcÿ?iÁΐud?gº|ä'FU?‹ÕG|Æ?‰=|C›¬?îrñ?–ä`v¿"`?'îà{ˆêþ?~••¦4?¥!eà—uv?'ԁ$—^ã?îT½Hq«?–þ¹úz>'?SيA*Kg?VƒU8¯\™?ªc©œò?–ÑÖÀÏ:&?ïÔˆ!™z?ƒ[í`?GJà¶?X[ÚR¼?s
&æ‰?@6T¼w?ïÑ>NÍÌ?r‹a"ÔÉ?Uû¬D%M´?Qê¦ÒgA?qáíá^°?pLC}•Æh?ïJ·Q÷º?[ÆÿöX?ü42¨o?l
¢?5m?ŒM/\Îü?wë9ˆ¦Ù?
àXÆ?us‡tpš¾?DÑòE>7ó?7NÑqû>8?‹‡Þ2Fý?u0 ŽDÄAGN3FGL J2041.7-3732@gE_ۇÑÀBš$€	À:w$ú‹LÀ;—œ`ô6ž¿æ«ªùÆÞ@
¹« éð?ü™Þ¸Ý'?ãà¶cÁ¿â·£??¿ä\ÓÚL¿ªwYƒAGNbll?ïÒJ'AØà?qñÄÉb?1wXP#Ñ?,=ßQ‡Î?uÃAx8R"?q´"
Ø>?ï…;öü L?‰"™ƒH?d.üæ¾?b2.¸é'È?‰¥CB±g?‡g"F컏?îsƒØ''à?Žž!?'}"GõMz?€æÝËFíª? 	Tš©=?†åV7mu;?îxûå ?Ÿ@¾!"l'?@b
+r"?Hü:È{ñ?¨.Æ8Ÿ]ó?Ÿ6eÞ$dÄ?ïòwDÒÕ?QûšÕ€½ç?#XWę}t?¿Út'L?X¦lÌ>*?QHì/ϳ?ïÒQ¯­?u"Òy1í?TQÔpž\?QÆK#"?qÂýþ±o?r´Š¨'am?ï^gM}H?w*¢Cû?ŒN¾/I?pxb(ÿ?†ð×^š@é?hu뉻?ï³.?tMtOL·E?!N7U·®Œ?!·NÜ@ ?'÷ºÑÞ?t(#QíHAGN3FGL J2041.9-7318@t
ÀÓgÀ@Ýn˜K¼À:¬(©lÀ;ɨÛUüŒ?óVµ"ö@Ë$Np@­œ€~Àz¿é«-ˆ×Þ¿ëM‡sb‰s?»fpѓð¿âw ‰s—ãAGNbcu?ïG8gßI?žŽàÀæ?g"W§±X?q1:	ª?"&"Füò7?œ¦øIIÂc?ïžkC"?›Ú'vÿT£?~?
°öÁ?'øÇâ?w?—üoê®?•yôåOž?ë0ß¾8'?ªmÞÉl?®ákJ"Ür?œ¥o<?·¥ÃZžŒ<?¤KA'‰"p?î?¥Š3?«oä±­?…ï¥ØœX?™Yx´u'?ª Eƒ€Á?¥‹få ?ï±±üšxo?–¾ßúQ?a™à9±¿?eÊ
恮ˆ?~Z¢I€y?OÚG""ý?ïõ€,5?"úº³
Â?sK~çè5L?‹BbZ?'Üþrà?ƒìÇ—1?í‰DÉwq•? j—ι?¡³ô—I»¾?"7FšŒÌ?¥·¾Òöøé?—ÕuÂ¥?ïPÄȾ•?ªK#²?‰i+C£äc?ˆ°VìÃ.¶?'e¢Š›²H?|(¿]AGN3FGL J2042.1+2428@PòaßîèÀ%–Ä!, rÀ9ÓpàÓÀ;†3çÀ½¡7Ì¿@Šþ@8ã?ýß#ÿŽ–¿ëi*Ý4Š2¿Í'«é[Š¿Ôjë%¨[(¿Øb' 4AGNbll?ïè' «F??hºSÜÍ?AõT"´0"?@k"µ)ÔU?c[Š•\?eg¬™Fÿ–?ï;ŒF¹'?œjlšS?s'dŽñZ+?~&'ºF?"·õTtY@?—£H¤FŒP?îï[3
!?Š°u¦Øë?‡ÿ8g¢?s0ñO9)g?–tùûNØ?"±›qx"?ïÒ0nç?sÜ'U>Ý¥ô"Éæk>çø´ù†—f?vàŒÎT>J?s¯Ä¸[?ïðaÙR°ì?j°¦¾³é?:-© {Ù?C˝@U¬ù?Xœy
­?f‰û©¡Z?ï¤ÜšÝ?Ž&1†Œ?d	GΖÿ?nxý¾™o´?Æ­/þ?‰RIÙÂó?ïˆÀEªÚ	?túD"ƒ?w¸ÇF¤ùÐ?aAk<\zF?óŠùÞÚ?p¢;'—Ó?ïõî†ÛÑÍ?IÈ3^9š>¶I3ƸÒ>ÀÀ•N™}?T_À'¡o?IÄ.m=üAGN3FGL J2042.1+0247@H?÷fÔÀ6ÿ n4'À:Y)ªIëÀ<:&1Âð«?ù)Õq6#(@
É, ð:?áçy©í­¿ËZfØ1¿Õ!÷'"b·¿îOÙGÀš ¿ßk;Õ:¦çPSRPSR?Ö-g8sd?Ñ9¢N0?Ó(8Èb~?Óþ•»
?ÖªÄл*?Ñæ¸o·aÅ?å£"A¯‰?ÔtÓçsA@?ÇrU…Ìì?ÍX²\ՙ?ÂMïps?äêÊRÛ?ݤ«ª'
ü?µ@c¢Dl?Õ|吵fÌ?·8‡$ßÎÖ?ɼ݉'q?®§†ß[.u?ØÀÇgÕs²?ÍQö< ±?ܟR
ª?ÐÙé їô?Å?Í,e†?Ækâá%
D?Öq+àÈF?Ò&M{LÁ>?ÔÂw":+?ÖٌÐÕ½Y?Õ¨»?ÒeÓµZ{ˆ?ëâyqÛåo?Ëàeþ.+?²Öö ¢Â?Ã3˜¾}S¾?¬*|¢µC'?¸œÈòÿdÅ?á6êìX¿p?µÝ™¥ÐV?ÓQ¾'ÝŸ?´Á²_Ü?ĀØyG?«ÓдÿIÎ?åM:s{w?Ãj=jd?Ò'¼2±ê/?Âv>å\Õ]?©îw8è÷?©^Ñy]M´MIXED3FGL J2043.2+1711@NóK 'ßÀ.šDÀú0³À88í¥,uÀ;I»	Uê@¦óp.@Q	@¢C@Èx»¨'¿×܀"'(}¿Ýk'oŸcø¿à«ƒ½u}¿ì«Àã†PSRPSR?7ƗˆÛ!?‹%ïò¤tT?ï]ÓÇà ^?Ž¥÷¸î$Š?p7¯¼ w?h¯…‡r‰b?'ºéÆ?«ÍººÊ?ë=Òýy¤?À,|É<—?ÀÑsÌ;¾ƒ?¼H
œ¬?¯[*);'? -NÖr€
?ì‹Èº]M?¥ˆB
d?¯ÜM²O?—‰ýÿ¦'?¶Ì5Hc!?¦-Ëî•c?é¨âôpC¤?²´ PÔð?»ì³Š˜Â?ª憑'?"r"`†*b?˜Óš,t?ï"~n3Ô?Ò£âƒÿe?i·€S²7«?iÙÝe¦ý?œQöãc̊?¬Æ¡Oö_?ësâ=ªã÷?¿	K
ó׆?½Lp[‡» ?¹N`5þ?½‰"E?¨fðv‹|¿?êƪ™q*»?¬'
ðo?©ŽCeŠ'M?—r†2É&?ÂߣkKõÄ?¥r^ÍWñŠ?闳³Ô¶Ú?¨§/ÑwD?«7<‰S?"fü|S=PSR3FGL J2043.8+2741@Q¨¸!ïÀ"NîÀ¨tÀ9*AÖd%DÀ;ré?û1Œ$;¸@dóiï‡ã@4J´RE¿Ö…<6ß\"¿àú¼Ê J¿êia@óÌQ¿îÚâvy¦WPSRPSR?€[GK^þ?ƒÿóM鏠?ï€gøüol?ŽìÞ6Âäà?uu1Œ=?Ê-TÞ¾ç?žßµ¤ëq?–ôea­?æSkÖy4?ÅPÀ¦'•2?ÒO:Wa2A?ÄÞ¸z¸áf?µú:2õ®j?¢"ÅG½ñÍ?ê4A‡xž'?«™˜EpGr?¸c¹'ý+?¢) Lçl?µ©^ãA+º?š@{§2ŒÚ?êK(›»Ã÷?«-Ä´O}?·ý\<ºó?¤_ܓÒì?¢ÁK¿Ä?¤W´´•6?î[DG~³?©í9ßÒ?Ž*Îr¯Ãÿ?Œ[à˜µÐ?¬¢*³n>?±¶q¢¾¤?åìÚ»;Ė?Á¿— (Е?В2'D-?ÀêÓyus?ÓGef®'+?³ã9t
«å?ãÜSˆ=PÃ?´ÒÚ®NìÔ?³ÿÎ%?5?™XŽ¿ÿg‡?ÍIÓ;Yzù?¢øØ²?撶`@?¦NÉxž°?°Ö¦Š˜Ê½?˜Š¯¢Ã¯…PSR3FGL J2045.2+5026e@V06â—@®k³¤ˆÀ7"S‹˜OÀ:C/(·Ä@¢ó_2•@G™E`Ý;?ýÆøÒ¿Ï©0&Ž¿äùÄ÷k¿èƱ?R¦@¿ìÃ"Ê/c›OTHERSNR?bšÛýi:?dе‡_£?íÅ=T|â‡?³÷ºyµŽó?±AD^wÜ:?³§Õ1ûC»?\8Xÿn?hÏ:ɖt?ëv¯Uˆ?½-[F¼kÅ?Ãu
Õ,S?½*i1ó?œÀ¹òi9?•Ke÷.3ë?ê%ô¼ˆ?²šOÍÍǬ?Ãåôõú‡_?°á"¶Œ2?~­Ù@Ecæ?sôN>°?ê@¼ŸÇÊÉ?¬ì}—Ñ?Æž¶J:?¬0…wÜW?V®žB.¦l?]5ù¶¸¬æ?î¹o‰"'?¦¦
®Ÿ?£³'u*Qø?¦ZŠÎÆ9D?kâÌöÌ?zûÕˆ7?ë—x½Ú?³Ù°õ{£­?Á4–ô?³öfðo¬? úßåõ‡?šŠÞe²~›?êÝW¥k?¯$öǁ7?ÃeÒޚæ²?«~7*ž(?…Ú–vêç?uÙ&z"½é?ëÑ¢­Ñ?¢ˆ'•o^?Â7Ž«‡‹?¡Æ[€šŸGPSR3FGL J2046.7-1011@Bl@%NÀ>2w"^À:jSâÖ#ŽÀ;"bۗjë?À'@"ɝ@ŒV¹ E?ù¿WAï9?ïðª(¡Î‹¿¾½mÍx¿×."Â3/œ¿Ï$ô'IÕAGNbcu?ïöJ#"?G©qbǍ?.ý´/ÎÍú?(&ú몭U?OßiÃÇo€?Eróe¸´?ï:?"w?¢ãÅ6ÖV?rÐèv¨â?q±'ã¯pP?"üWcp?›µ‰VƒÙå?îªj.ÇéŽ?‹ìtàŽ?Œ½Ô…—?|þ"Ú4´Q?œSÏÝcÍú?…k;'q??íNÊ-`5u?¤n©—Ð?uCQÆi®â?wuì6c°$?´5yxUÀì?£û(½©èH?ïùÏgóŠ?=J‡O,Ž?!»SÌøÞh?^¯y­³Ñ?DSŽùæC§?9öÏèöÈC?ïÅ'}Â?{'ÁŸ¦š?^Ïåå.cÝ?]4òfiŠk?u½½¸Ï>=?w¢²±"lv?ï_Es¸Å•?x^nU²¢?' PIóÚ?i4sEu?ˆeRñè°Æ?sg"ó?ïGCۙf?'Z@È-?fŽ€­*Ã=?V>(AV#[?"Kgt'ÕÙ?û¯ÄE×AGN3FGL J2047.1+1054@Lˆ)³únÀ3¦Ÿä6vÀ:\l6‰ÿÉÀ<,)ñk?øyȈÅ`ó@-zØcXë?æʒéYÔ?îËa¦Üi?ÄOð Âv¿à"¥…¾¤¿í¶™£ÄY¥PSRPSR?³µS8=1"?ÀÄ	*‡NO?í[4¯	B?Âø½^£W?Ž~™3[6?œ"ò¹wY?Ñçåh5Z?Äk$¦¨uÕ?ã³céŵ?Ì	ËGo3?Í ˆt
òU?ÃVlȆc?Ê>äÞ!Å?´ú]þ³°¹?åì,ï!`x?¸ÞG"µ5?¼ ÎÆeï7?¥úé£nÅá?à/
Ò?Æj
êFÃ?܏™-
)?Æ«.u¹?ª¥
f
uû?ª¦›ññF?²™®šæ?¿øT Ú@?í&ö}º?ÃWñ%,O?"þâÀ÷M÷?¦Ýè?N\u?ÒÑ¢C%2ƒ?ʊGׅš?àìg,'¿?ËA9C×?Æ«Çkcü?ºÈï­à£?֙æmT8´?·"ªá·âÒ?â›åƐ??¸¢Vž]¨Ç?µs‡§¸?£aˆ¦Å5±?袈ì?·hHOæLo?Íbd¹"	2?¶.(7zÂH?'leì´lÛ?'[2žÞ‰MIXED3FGL J2049.0-6801@tj‹@p2˜ÀAò¨`úÀ:%êIµU¸À;Ä)Ĩb?åæ)Aí¶&@!Úi˜u@xÓ@Yap¿íƒ˜í»ô|?ÐìMë	<®¿â§ým‡¢¿åGqaIÐAGNbcu?ïöþ"Ÿ%?JO²ïRÒ?@žÝŽ\_??""¦…»?Ch™º™Ã?@jaH6í?íù+Í/À"?«§£šä"?'õ\°QŽ_?–ñ~'?"Ï?§r"Ñk"?¥ûoÐÜ÷ž?îÜ	À•~N?‰b©˜jE?ŒmÛñEª?{˜@Š&™?–GÙøL[?µ8Ç?ì5½d'""?¦õ¾a
ÜÄ?±šÐLõVM? Œ½G†˜?©n‰ ÆB?Ÿ—¾õŠ
y?ïü&Œå3Ô?4ž¯œ±Í?&Ô/jˆÆ¼?!{»…^Ù!?3a€Ï¿Òù?-k¸"Óë?ï^T ¯ý"?8OU<mP?yµ¾ÓŽ×¥?x¹Ñ×Õh?‹ø[¼?‰Üõ¾ýd?G@Ë?y€ÐÖñ6?{Øωõr—?qH¼÷]•@?ª[\DÁ?qÅ	Pâú?îÆ}zª=?ŠÁIÈO·?š`4œ_‰¸?òG'´É?‰ 8ý-o?~û¿ìyAGN3FGL J2049.7+1002@LWú€d>nÀ4­€'ÍÀ9=A&QÀ;|v,­5?ÔSÑA@j•pj @9Ûm¿å\'"Á¿æÑX«Eq¿åÇiX¿ç‡ëÕ·¾.AGNbcu?ïôˆÎ£Å?P
t£'?:ăÒ5µØ?7«¿m'ÑH?P=Aí#£ã?Ko3's6?î×M$(±Ù?¤¾~ÒÚ2?'ÒYÙ
A?ƒ¥oó&*?›­PÍÑCO?¡û'ŒMðh?ïá
=é?'­:X|?†nR؏ڛ?riÐÍ98™?"Fp¸‡˜?{Þ´Þõëh?픣YК¦?›¤¹)Ï(¿?†Kiñò\e?xÝóÌÒk?°'wôÆ>?š}'ï¦?ïûD0¨á­?=çH"ÐñÕ?/½¿3-ÑÉ?3L'©"#ë?5ÿ›š€ÝÄ?1÷çáàF?H춀?ŠUŽ	Àž?ižÖÞ¶;¶?dš'Ú¹ý™?­ø+s?†ï;q!(º?ïšíð;šh?kBÏ®äx?unv¨¢O?c]á wŠ?}ûK=՞?\S`Y™êÆ?ïb…¬ãßt?}Gˆ 
)F?ruiÐ/ƒ'?\ÐëºØ"e?Ž#ßæ×{W?{z½x(€1AGN3FGL J2050.2+0409@I·PÿÌÔZÀ8t-݉À9Ø
¨_/À;"8PÍx?ã<ð×v§…@
$*ÌÝ=Þ@‰¨f翕ЉÍô•¿à4Õóo¬i¿ÝmyzÀ:˜¿æÈŒ·€WAGNbll?îðäـ[Ò?›íeˆ?á	?€CLOHÆx?'ñ –ý—?™Á¾¡œå'?•þ‹³;?ëvxÏ
ˆ™?¿H½YÎc·?®Õ8zF¢d?±uØ®Ým?´áI&Œ?µãN÷{?íekÊ7?‡ýK+Ò?šÜÞ®DÎ?‰ÿ†¿iQ?©‹9ùXÃ|?•
HV¦—é?ç8ö…q³?«{9~ž8?¶.šK÷ùl?¡¹·ëÿ?ÈÛÏ%6=?§qnÿ¨qm?ï¿¡¶ÒB?|›Äž­?[·¶]0§?aÒ*ªÜ‹©?yA6÷ýîÔ?uÙn®üÝ­?îO,§9%¢?«÷ØLz
?•ø©j45Ä?˜Ãô|L? àÔ¿Ö?¤ßɎ/×T?ï4/'#±5?}ñ0ã"k?…ï#sSˆ?pn¹ÀÜKÁ?ä0LÁ'<?u¸›š¬:?ìmé¤Á7e?'/cz5Á§?«JÑ '?†"}s`Yc?­Ö"™!%?‹f ‰RAGN3FGL J2051.0+3040e@R¿íÁ9À! ÀŠÀ78IqcÀ:ŠÂp@°1a÷ÁÃ@òäñܦµ?ýÜSûª°Ã¿Ðþ¯¾3G¿ãlˆÌ¼¿åSºÇ犾¿ëÈeÊ_4COTHERSNR?yH.w¡Ÿ?wEÇD¼?îÞbœŠî9?¡ìü.nG?íZ[Í"Œ? &õ§ÖV
?d׌Úø–?{ØÌÎdþc?ëüCrùû7?µÐñ«-´§?¿w+›cÆ?µ˜ÏÌï¼?¡á¦Ç¬0Þ?– :ÆÆ©?ê¬ ɒõ?±|éD-ª©?Ã8åË\›s?®ÙR¢Q]?eß2?ÕyÏè˲?éfÑÿXÊ?®ˆB:Th?ȎZ.àØ?¬ñfJ$?x±Omє?€lMVi«?ïL#¼óÜ?'…¾Ô
ID?O4uÇe+?/ÎóÈ®?q‡•Îowz?|Cnj½Ye?ìHPŽÌÝ?³y€:‰$?¼¥-Ãd?³;B«-J?´¢ÐY\-L?¥â"Kaz?隆"û
8?¯èáÝ(…G?¾ˆû€ƒ6ð?¨šÎ=Ôç?˜¬Àêu½?ƒWV¦DjÆ?ê=@þ«tÁ?£Èôd¼#O?Ãõcç'Ž\?¢XïÞ´P¶PSR3FGL J2051.3-0828@C™* dúVÀ>v |wJÀ:yö£•œÀ<FÁƒÃn?ú7¸ék@Ë»O†¦?æ¨Ì]Ÿ÷?ïÿœ)''?ÅýíÍž¿ã4Ìå^¿ïÿMfÿØ,PSRPSR?¶Õ¼ë-`?¼_Ä-8j?ë7[mR؄?ÆÿÊìÞ÷-?®ÞÏR¿é°?¿E(	Ö»?®ÙÀˆU?¹))'Hi?ç‡%8Ò7#?˪ƿ¹á/?Ê,úùŸ­t?ÅAÂ!UÄ?Á#ܾ‡d¹?®!"ÜÆ6}?æ'ô°°PY?¶,ÕV¹>2?ĐP~·Yã?°!…+Œ?зò#<®?Â:Ÿ\Àäü?æpÑۙ2/?ü¨×˜?£3Q(K)?£"36Î?³ŽÓ¶Ù˜?ºñ3§éÎ?ëÙy'ð,E?Äñ©rL?¬KJ(³¡"?»LDH¦¯N?Á(âù2†?ƪ‰zj=?æWøxæàc?ÍÄöнƒj?Åw<kKí?¾˜ï±?Í?Çx'ù?´nS|3?8?äú—^3š•?·
9ÈÄA?½«¶,g?§Ñ›Z[›?âi¨ß'?¾ì€­uª¸?Ùóé5'?¾­tSH?"ŒPÏ´j?›<Z+ù
ÌMIXED3FGL J2051.8-5535@u]Ø`fÀCx) zbÀ9ÔûÔ!TäÀ;¥°a\;j?ÇÞ¼Eb'#@ã'ÎQ@ž^ qº'¿ë ™¸Md¿çúË¥ÕE¿ÜqtAEo¡¿àGŒ5zW¬AGNbcu?ïû`kz¢^?F`dۇé‹?rÔfòË?ý²h¶e?@Oöè>br?E'5¿x¨?ïŒ÷7«?"`,¶ýb®?dÏ:îo0?fÙ'ðP1á?‡Žcaw‰ç?ÁBÒÐÙ?ï°r	mù?†H;u5?®Ý"»~‡?n—OÃÞÐÔ?–''íéN¤?ƒt€í:ªp?ïf"QŽÇ?…èƒv<~S?B|?܍¶Ÿ?E+ž™ŸÐ?'«+q°·ç?…}ø7æt‰?ïûÒ¢z²?pvÀ30ãÞ?F¥@­ë?Ž9?½)—?>â,'¯e:?pu'üEm?ïÚ})eC?nQ´¹Á¾?PVQÃ.¤ì?M–3VnI¨?mÀZ/lÆO?i?=ԁ?ï¤I¼È®ì?n×úý0ž?oamU0o?Zä;¾œY?~*jçqj.?hÚ"ÎòI?ïàóÉ•×?cr÷ë§-?9ÏÒ%øhy?/DsÙ]Ø7?kÒ<Ðü>x?bw?u¸s6AGN3FGL J2052.7+1217@MŽnß±«ßÀ4ù@ÉìÀ9Á+KÞ$äÀ;˜†1		?Þ"ɘ\O@
TŸãŠ©@¿ÑÔ¿àÍNnðE¿ãQ'KŸ:ÿå4'౟ä¿äùÿäþ›PSRpsr?í6úÑÔß?±(ª~è?#?Ò!Zûœ—?}}º<ê©?´K]"ð=?°xA‹3Ñô?íõD?½ÜÌDø¾©?›³p?¢*¼ðu?°w–9$ÕF?·™À²Š¤?ìÜ$U§?£ã²,£Q?œy
‰ñ±?†sÚ5?´bÛ"âÛ? Ú	÷e?çwÈOƒv?¬Žëµƒ©?²Úƒžù"?¢òi1¥r?ȳž=b?©sE4ý´?ïr¨Â½€?'E×>"Žß?c¥UT½;ö?dNîGæÜ?ŽlyôåO
?%ÿ'¯?ï
!·4à?©M·ò3ß?'ß>¨«#?‰»¯í_?•L)Ã*´?£Ã¦µ]ü?ï	nLӇ?"úJH‡?†€wëÇÍ?v–N›LÎ?"'úí0?o?}f§er-?í,?ρe¤?"iÉýw€?¡uwu?…W;EéRÆ?¬5é'rŒN?ì^›=tAGN3FGL J2055.0+0016@H9Ÿ C×ÆÀ;
v_Ø­¬À:xÊ J"cÀ;ž‰.‹C?)ÃZ<¤c@úׯ~Þ,?ûºb&%Ú?ïô>!gž¿èþúÔÇíë¿Ú°à¤a
¿›K§7µ"AGNbll?ïÖ5ÀŽ¯?€sp0a)?#2=—oR?%DE€Ñ[?tKŽ&$~#?€býÁXoÄ?ïs}ÎaøC?O<Ь/'?ohKd ?mÖ$^Vª?‹[òNy{:?Œ¢£Øâ°?îŽ'"XÅi?Šµ/²|?ŠôÀ;+ë?u`'VÒ? `]Í`|Š?†ür=xã?íÇðԋT?¤Ž5®ÕÄW?P‹Çi£—%?[">Ýãe?±~J="æ®?¤"Ö: &?ïðWükJý?d±mù?÷ÀyoU…? o|¬?]p‹ï$?cðjH	ºW?ïÐ;‡±¾?q¹­¢'Â?Wãy
gYœ?Sc.Ç'?qé^)^N¼?nXóz£A´?ïZ/בªj?xµ"B¯¦ñ?}ÖÒC^‹?iù:",jW?Šˆ ú–F™?qƘv2$?ïŒÖàvø°?~s¥ŸznÝ?DÔòï0–‡?Hëa'"Êß?‹|øµD+9?}µº¤è•sAGN3FGL J2055.2-0019@Gó¢`¸À;hT`ªdÃÀ9ïtŠ˜À;cÌütð?Ü —8°•@hcJ?ùÿ!@AŽ–?o=òÌ¿¸íý^C¿Ì®ÅG>пÓm•¿ÅRZAGNbll?ïæԖ"tR?^Ý7XÿÇ?@\à˜È©?:ÕÿùÕÉÛ?eBˆòM?[°|ÂmØ1?ï3Ê–X? Œ;õê÷\?yÙ[þóŸ?…õ±ˆÓ˜?"h΍¦£?
RíÆi?îÇ^rjðS?‰'ù"uL?Œ"¿´G‹?x'Ç»ði?˜ÉÑÜmá?""©
׎?ìS1¤×?§áSÅäv?^"_ì?€%qO2Î ?»p‰•jŠã?§9ìñ–)?ïô¡À¸?JÆ´Ž™Û?0í?xÊ0E?-öOŸÛ?R/1P ?F\šU_û?ï´	óQyx?"[ÁUúû5?cžeù\Œn?a<_*'³Þ?|+ÓkÃ	º?'(¬_¹?ïrZ—jC?w®1ù½?€NQ…g?p¬k­Fû_?ƒM
W"ÿ?m—˜Õ§Ñf?îÑásݍ?‰/+–П<?w†&ãØ Ð?esuž·Ã€?ŸâGæÒ5?‡ºß¶õ¥'AGN3FGL J2055.8+2539@Q¬iöZeÀ)
¼ßÿ«À7 Ž]%uÀ;=¸·a+@~ÃS&m¨@JԏŽÔ?ûÄwÌk¿¶ÖĪ5ël¿ßc–éÍè¿éñ8‡¹zé¿ïÿÛrW
~PSRPSR?c7MxF¡D?k|˜Uñ?ï©ÏPyƒé?Ž*`ÛõÐ?€¾X"•?\?‹â,ãìV³?^"_³ö8?€¬½×Ÿ5?îþ¬1»~?¯/]Žò|?­ß+‡ñ?«]}ð¬â?šHNÀ…Ö>?Žñ½›L9N?쒼ª.«ÿ?£o}¼Cg´?´Øýû6û? ½õ¾d}y?BVÆZ²?KŽ"JÇÑÛ?ï»zè(Ù?y'åG¤Ÿ?€˜ÆåG?wþ‡ kòw?`u2yRf?k'n?ïŸÛl''?'hùa×ë¢?"2+ѶÐ?X!1Üyœ?bəz†¢%?tƒáªn?íð#~Ù;?§ËyPþê?¯Ñ."˜m¯?¦Ó¾¬¬?¤˜ãÃÆ?™®BÇE'i?ìhYJ
?¤×âè»?²scTš(c?ž'Î×»?XŒØÌM‹¥?J»F­m?ï¯mÕµB†?u<Ðâyf?ïröa?s³åô³ÀPSR3FGL J2056.2-4714@v	k¿×ÀD0½ßÉÿ"À7HErÐ×ôÀ;|ê6j?ûü%íûE±@2ê
$@©³ûo¢z¿áO,²]r¿æ㺠^Ö¿çºg΁"û¿è;¤=XóYAGNfsrq?ïëÖ°ÙÚ°?\ûë˜ÚJ?XÙy§5Œr?W2¹ícŒ?NòJæd?L::SÁV?ïXÃ:§Ç?‹¹¼Ýhæ?g€gr˜·f?}2±\ö§o?†IµD‰¶'?'©Ãî	è÷?îÈïŒâžh?˜tzkÐ	x?"¥VôÕëµ?'!ê
¯¸?'<·wmMJ?[¶ÎÍqÒ?ïË1'À|?¨ÎÐ99?@­Í¯èÂ?\±üÑ¥j?xQ"ÝjîÒ?@k"ãWÇ?ïõl‰sº@?R¡Þº±µ?L3­(Ýç?O"gž÷?<4Y|Ì°?6`*¶W­u?ïØÛK?Äf?n'¸#È\%?RËi¹6€?R…Wh׺Ô?m¿4nŒ?gÖ¿Õƃ ?ï)¢,,?'"àg¤Î?ŽÀVùŠ;?Šn]FPH!?‡*—+ Ú»?'¤Á,½ó ?ïõ4§ý_'?_UŒÙªœD?-â;'?›5?98Ð-?QÚh·¢˜?^5×ÁCAGN3FGL J2056.7+4938@VSI`0Â@@ô´À;™ßÀ8ÖéÆ×qÀ:ågÉ<õT?é
"v"ÜÆ@[uLj'?üˆH€ø8¿×
Àي±†?ïýmaw¤¿×:CÀãϿݨSíN2ÏAGNbcu?ëÓ'"Ü…?ºùj¥nˆ?ƒ??íÁ
 ?zOf>gã?¾þÛcy³0?ºv†,:­?â‰61ë4—?ÑÚdPÀ?À?þ¹•Å?¼S³à†Ô?Ò͔?_ð?Ì6Yã÷
ä?çø--­?²Icˆ¾ê‡?§Þæ\?"`©Í")
?Ê(KeP‰'?°ñÑ|Հµ?á‡Ñ›À?Âa!3'Ë?Ò É*Î,@?Àtí25K?ǨNc÷\?À	èŸnÎG?í7€9Ì)?¸8*Uùc?pF(†±?ir ëõ<q?µ?ž s]?¸R	Æ<	Ó?èC³@{à?ÐHê'Ѳ?µ•¾ô("·?¹Ó]üÇ?Ä&T	Žìd?Å+gd	·0?ìÍ"`kê?¤fïkeÝ2?œ'éijÆ«?Œaà۞L?²l"â'?¡N¤"æ]?èE;öT?³|Őêß·?Ábn+¤?¦-n'òË?½
Fµ'??¬úkä§nAGN3FGL J2102.3+4547@UÀÇä¡Ö¿à	'€4\˜À9N‡"žyÀ;˜áãµG?ù°Ñì~@¡/Æl5ˆ?÷Kc-vÛª?´  S¿ã¯¥$W¿î£#á[¥¿é¼å~tz%OTHERNOV?îقçÎ|?©=zÃl[0?‡¨Æ÷Í_?–ÒÍg³_Â?˜û@­ä?¥jÊíq?àQIŒn–i?؃—L?¢o@äþp)?§XÚåþÈ?Ý"Ë^ì'?Öò³ê[[¤?âæ7…¹y?´ó‡âz¥?ÐȆõ…±?±Öa¡à®å?Ä7Û/9?¬ÿ@"ÁV?ï"¹òï:$?™yÒ°‰?{"m¡^×?"'ښ)ß:?"Ãæ;Œ1Í?—R\,÷eð?ï1dƒ@?¢¬§Ãqçö?'Š24Ë?—_Êzhû?‹ð'…ÆV{?—iý©]?è|wµCCL?Òö,¤p.´?nT˜ôÞ-?¢É™@Í2u?Ê`V—fcŒ?ѝ™¥ÐV?ä6Ü÷xƒ0?´sÀžÄc?Í'E(Ô	­?±4XIE­Ú?ÁýFùIé"?ªÃˆQ.+?ï¬3rk?†)Ÿ}☌?s!¸à§b??yòÆ%O°?vÝÆÿ@n?{;ýK«ºAGN3FGL J2103.9-6233@tË¡ ÏÀC{+ŸÀûÀ8è_⾦™À;em¼Øc?é90&³Û@Y–ù+O?ÿ›I?2É?¯Lùû%¿â¥—\[(M¿ÞLYy1Þä¿ãEÊ/ŽŽAGNbcu?ïøØÏ›y?H¹¢õè…B?(+G×Hâ?"ø>V¨v?F'ñ{g¿?FÝ»QŽ?îÿ¯²­Y?¡
ۃÒeœ?Ë]VYS?'7^Aýñö?˜2c¹ê›?™ëÔ¯,C?îý/÷ЗÄ?‰ôPXäÇ?†k>æZ?yÎUGãùú?•Kh1Y?"dÞ|¦²o?ëñ,¤4
Š?¨#ëÝ'E¼?Ò·6Qd?ƒñcäç¯×?¼|C÷•g?§…©"çÂÂ?ïü«¥ñÒÒ?0´
¶Ó
?!Wÿ
9Ž4?ŸDþB:r?1öÏæ7G?(²w–?o?ïšYn2…?‰]	ölç?n֎:Â}ü?sÁø—-¿
?´YÅ4?"š$ñá`?ïŽ][®Z$?wÔóaáòN?xIñôaÚ?k—¨'yà"?€DŒ1?r'·—˜Lç?îÄ%Ýñù?Š§sšIâ?…gúNàï·?lÌN‹1?œÇG/r?ˆÌÂ+';ŽAGN3FGL J2103.9-3546@aåéSÀD³, zûÀ9tÀ#i'À;§ò¼JžŠ¿Û÷øYÃjÎ@wçî@ç@GD¿ç	taÀ¿ä=t:ö‡¿ÛJÝQ‡å›¿ë²æë´×AGNbcu?ïðBj*7®?`ñZÆÙ?R¸mø´È?WñHTÊ?I…zê7Š?NOe«Ø~u?ï{#?}Ìè?z
9èÙ?lŠX•¹¬?|‡ù¯ìÓ?Š0
"?‡?"Ð6CøM?îLþ	tŒ´?˜¢xâÖ(µ?žÉ¸d?'ô€b>x1?˜qJŽý0?‡®â+-Ö'?ï"0(¼·¬?€îfH¡?@ÇUvJ{?A^bO¡ùÐ?Š2il|ÁL?€µÖ)¯‰@?ï÷î¶×m?G8v1E"?E¦í]Ç¡Œ?A–ŠmOk?5<lԆµ²?24˜Çúm?ïÓøõ—Î?q%ë(¯Û?V¬+ªnL;?TÞ$êlY=?pXz[	×?kh'y…:²?ï:Âjs?ˆRô*?ýáïSx?"0*†G?ƒQƒiM>×?wQ2å"ö›?ïèξÒ?\aÎÚ3h?+71z5x?1Ó|Hrhš?e}ÎN
†¸?[ZH[Ȃ'AGN3FGL J2104.2-0211@G°l_¤«FÀ>Hï 6kÍÀ:­ƒðºèŸÀ;²/ãšj?èÄàåç·@$+"Ãyg?øbIÿ''ì¿î86#	ð?ï²ؖO?ª¶Í±ú
£¿Ê]JÚùòAGNbcu?ï루Œ§?c`_e)?AbÖgXTÊ?@o	u-?`+ð1Š?a¾Ý@Ð?ï&g	›×"?˜JÀyŸ¥?yóâTI˜?'_~¼…Ä0?"¶&7å.?•$(›ƒ?îeot‹\?"¨dƒ?Ü¤œ‡(¶?'.ÛÀD¦?¡±å¿Ë?`oEKþJ?îgÞÉÆÕ?¥|ø$ô"?²¯'ÝË?'ªÌˆ<C?¢#=ã3˜=?¢X$
¹A¤?ïñ¸ê}ô?X÷JZ?6"‹J'?4<FüÉ?XH
Y]«?U9\p*ùÁ?ï¹[8é^1?Q"}ra?báFžûN?]¹p«b«?zHröoÅú?z³…²í·®?ï+Öadä?Š0ÌÏǖ?…®³]ð3?*‡cDF¤?"C+}ü?‹ÆpT`[^?ïiÃ5Ê<?"7€ègÇ?…Dpm1x÷?{u5(Ï?€v¶íœ	?yò"‡1AGN3FGL J2106.1+2505@QðMÿÒ³—À-\n>¡ü?À:íA·ZuÀ;âž43?ØR‹!J—B@žo}¼Ch@8©€—j¿Ú‰`&x:¿ë9¤@^p¿éV/3¿Õ€ùŸ¾¡¼AGNbcu?ïà±>.—v?q[\É	îÉ?W/A¿›"y?c•Òð"[y?c· Æÿ˜N?fR1b¼ûV?îî!·ƒï?§Z΢wÕ?l2¤1>?‹'Ì"ÅT?™…¯Ê$?£]!"þ™?íçŸ3aO?•…ß"Óü?˜†ÏU?ˆp
Qû?¥C^ð¤Ž?LõÝ ?í['8u?£H±"u?€£h"¶¤?'¹*ž9é?³y³¹ð?¢-Âçðì?ïóK+ÿÎ?gNÝó5£B?9j™ŒˆÑ??œƒ=[?S&ŽÂuà?e–Ú9TYþ?ï±ß¸¯*ó?ƒÛà|´0÷?cv&ñ+$?dóÅ~^³Ÿ?}UK$],?€
ßKÔ?ï3¹ÏÞ¾×?É-¹'O¹?…^ê­C«¸?u)IÀŠi'?²¡P½Ê¶?z
äAÐ_?ïm﫸ÄÇ?}ß\àkf1?i;Îö
\?`Íÿ	Z{²?Ž5!FY?zè€x["zAGN3FGL J2107.7-4822@uîâ@1HwÀEéÿãzŽÀ:Ú
'/ðÀ;ª¢år¶¿È¯!²x@d
"Íڔ@°vÿeÑ@¿êÎ+‡ ÑO¿ëyµbÛ¿Ûý裗õ*¿Öû%¢sTXAGNbcu?ïï¶<@&?c-ÞIFÑé?	ñ<­»M?#þw"'O?^òé½¹Š?b¶ÙaUéj?ï{Òû©ÈÖ?	Øay™?fóŽM«à?h¡'?Œ?‹N]hãY±?‰$el÷?îøƒ‰âÂ?—ÀK9XI?ŽÁqł:?x"Ìs¹ž?¦Œo;öF?"7Ο÷ú?]'q?"Â7º¯Óh?M¡ÌD£½!?V¼Í@/.?£ø¾ç2³ï?"ŽÙ¯Û»­?ïøùªÀ!]?KErŸž?

g…õö?ù±A«§þ?J,?JgŸE&/J?ïÓÄ!Fe"?q'Ëàça?UJ³æ—?TœI™ödŒ?pËB~¸(?k°œ~r#?ïQé|Jî?€ÅtŠ1Ää?zœJ?a[Mu(?Ž{4š4 Ñ?~8¼
¶?ïÁàŠ\?lö	™HFY?AÍHþ?5s³4ti?|í¡d±]ð?l3"ì\éAGN3FGL J2108.0+3654@TF= ÿ:À،` &;À9ûì_9K{À;8Ò¯dÝ?Ú£D¤Zú@
ŒnPzÂ?þñæ­j1¿ì¯ižª%¿Ò
ØznÊÓ¿Ò8ÁS-4Ó¿Ýäî–VAGNbcu?ïp¸õˆ?•&*(uÿ†?`j<¾&Â?bÇÝ(¬rí?ß0!'èN?"ýlm_«—?êJ¸ñý?ȖFnàn¦?e
{]?ŸÄâaxYÈ?Ã+Íž?ÅÄJ>´èø?î/ˆ0&1?•è"m \û?'ðGâS?}—GõÚª?¤{"ÜxZg?'S¤bxU?í¿©‡3¡©?gËÞhÀ.?'¦ân%øº?'£Áe"°?¯[®ó
2»?šÍKú^¾B?ï)&"ê2c?À`þgÏr?K"7Žæg?S{…¢5ÞU?™þ"ª}}À?ÀcD¢58`?îAˆNKE+?¸>ö4O?…âAɼ±?"CÙ2[¨å?¦nê¬LGÙ?´†¥èZ½~?ïHj¤ ?­Ÿö?€âtK¥É"?kÀED·Y?ä'Æ?}6ÚTýk?ïLä™6D?ƒ?}Œ6³´
©?k]¨Vê«,?Ž¾\j»À?xyœÐ»AGN3FGL J2108.6-8619@s&¥?À	pÀ=)¿"å­À:¯º¨¦À;Õ"[tšÝ¿ë÷>$þ½
@|É®4[Q?û×à3¿Øm1Vd;¿è—t¡mN¿í§Ðë"6Ë?펨¬S|÷AGNbcu?ïrtJ«?žÍ6}`@?XIÕXƒò
?ZÂì¾J¤?8&O5w?žp{î+ú×?ï€h(;*?š""¶y©X?nŠÉ†•?ˆ‹ð‰v~?ˆCCŸÝ˜†?'<àÂ3Qø?ì¹FIݼ?¢£çÎC]?¤m®ëü˜?–b(Ó®ŸW?¯þŒµËøh?ž§z8ój?﬊;q‰õ?¶i"Tvž?
˜»Ÿ›ù?%.ь,?"ÃX™oi?­J/áà~?ïÌï‹"Œ?zÛJ1/™?CÙÍÍ/@Ö?E"…4H"?w
8ët[?y¢¢@Ým?ïÖóÈ(?~€Ùøm?Wº;n¹¹?iEEK½y?nîØ|	¼?r±1Èpbç?î[æð†Ý¢?•ªåcŸ÷'?˜hÃyA(w?%¿"l?œ^t+UV?Œ§k¿@È?ï÷­ÌŸ?Wü¼W>ÕRüœ$Z>çi:x(¤>?PÅá©?Wð'oêšAGN3FGL J2108.6-0250@G±$€	À?"›Ÿ-WQÀ:6û>ÐÀ;á3}]?à{@,Ù@
¡nŠLI°?ÿz 'z?îÖî&
Û¶¿ÑùÚ*Èy¿Ý0°ä+Ž¿ßF³u/NoAGNbll?ïƐ~yø?t!MÐ7?Q|™mI»}?N¤Á‰ƒg?xXšrréK?rAà†NIu?îÁ!¹ÊLÑ?¨»–ù¿Â?òâ\·i?‰Úzïa?žâWÎs ?¥¤úBHFb?îšh&'?ŒR ÒA,¥?Žûr¬¹¿¦?z´õS Y[?5Aԁd(?…r|‡*¥G?ìW'·™¤?ªU4……Êâ?™†¶°Zð?"ôûº×ô÷?µ£¼¾¼Ý¤?¦R˜Û
´?ïïH›¶e"?Xª"€
•p?5"%ú"2i?2'_Ï÷	C?\
¿ù²ô?V=nPºµx?ïmÜ|m9?‹‹__°'?l·ÓunP?r¹WÅN×;? šü-€?…ùÝÌÛW­?ïaÁv,'?u1ü×Ív?€h3ðóG¶?ieD,F±?‡'n‰=?nBáXÐ?ïÛ¥éÅ<?ŠoŸ5•<?†$<4§6?u™*5(;?''m*zÒÚ?…"r&Ö1AGN3FGL J2109.1-6638@txYÀe¶=ÀC"ÿ®¡iÀ9‰³Ò*àÀ;ª'	±¿ÔZ䯘ñ@Ô×cL@´ 06ª¿æÀøùÙþ¿Ú"Îl›E¿â;ŒÊº¿à–j»­AGNbcu?ïí'—i¤?Ud\hŽ?BéF}q?9†‡°mÔ?\©\•b>m?Rèž)€?ï\nt|Õ?Ñæâٜ?kù¼?œA?h£-Žš>?'ZªÖ%?ÁsR?îð"ÓÊþþ?‰"Žæ±Q&?Šzáj
,K?{ÍTÇ®†
?"±ôÏã<,?€EX4®9?î¨IIÂc4?'=ÁŠß6?dþa«$á(?a´Á²ö	?¤+…EÍà5?È{é·<?ïùšbcÄÃ??W4â@r?-1Aª1G?&—E½– ?BOé•øW?8(]|¿çŠ?ïÍ_Ó¾ó4?s‹çžBp?WO¹¾·'&?RVÏÄʲ?s|'¿öÉJ?qB™—;&?ÅJU?suËÝY?y0»ðj»}?në=@ÌO¯?
áwy=??cZOô‹_÷?ï°úÁ:J?qÌ_ÅZŽ&?KÅ9 \.?;æ1â××?'ü,ûzy?q}ã»ê¼ùAGN3FGL J2110.0+0812@Mş±áÀ9׊Ÿb0À9(µ)B©À;gS˜-ˆÏ?냚þRþ@3N5m=@š)€Výh¿ç˜õªf›j¿ß'<ä{®ç¿ãÐJÝ7ÂÔ¿ì†Ð¯ÝAGNfsrq?îö‹"ČH?œ9qùˆÛ?žªá«ë§?›c2p»?d$Túã?b«Ä0rkß?íølêT??¦Z;Œ}dJ?—ô݁?"àú+TÂz?¤ïêËDÊP?¢?Ê÷ø^?éö°ƒk?®{Ân?ÁüØÅËÉ?ª	¾m)[?¨¡"°hÍ{?—Ç;Xꩌ?ëϤò¬õ?¢ÄÙp@§1?¦Ðž[¨ÐÍ?"	·}Ÿû?¶‰>
Éñ?Ÿá]or€?ïMçnÓa?'))Èeò?"Ñ) ô?'ƒ@ÒÜÿ?X߀¼ÿ~i?W»Þ‰$
?ï"ò¡Ú?•œwÁîÒz?"a;Çԅ?}KB}æÑ?'ýb^?'6ÃèJø9?ëW
"¬ä"?©5¿·A?¼I"ÞôŠ?¦m&hÝT¨?¡ûü÷H1®?'§«
<?i
NŒ?†ÙP1BY?—wWô,?y
íG?˜{[Ò`?'TTY3NAGN3FGL J2110.3-1013@Cè
`:Ó;ÀA·q?Þ<aÀ9™,å;XœÀ;˜£Wˆ}?íjìÖ±@íÌR(—@±íӄø¿âœJ–|-οì‹ßG<™¿ë,•yT¿ïö©¤2-AGNfsrq?îù²Þäý?§k¾|îaI?¤ëÍÛô?¢÷"›<ZD?"I-çz?"Œì0=«?árÖÐöl?Å	ptºÅ—?ÎjÉ(äŒ?Â	9±ôÒ?Íh.ۓAÄ?½dAçÀÌ?é LœnhÇ?¯'Ájiç?¼×	Àâ̈́?¥hÀ_‹hÅ?º&'_õo??¡§Õu׌]?ז&¬€ë½?²¼4ÁÄ)<?ÙY"V€â‹?¶=Qš"zÓ?Î ‹÷Ö¡ô?²ó¦8£ˆ?îkàí2|?¡"Žƒ[¬´?žµ)†ÐØå?™Jê"Eã2?"ÎÕ¹Ñ	­?'@¾=ö±?èñ«ïT?»Ê~òVþ?¾Ù™àwŠ·?³µøÈCÊ1?¹™x¡Š0?¯tykÕ$Û?ìØaâ·ßo?Ÿ†£ºÞ!"?«ê@Ǎ¡'?•$pÝÀ?¦¡
ÐNí?"buy³n?æºOzDG?§õ$aM?Ë!ˆ®îH%?£ä)–Ä€?¹—'-4y?ŸmUÈþCåMIXED3FGL J2110.3+3540@Tå€!ùOÀ Éî E>À9­¸¨RšÀ;kŒñëjG?¨—VrxNŽ@çêô€@(WÀi ¿ä¼ó¢	æÅ¿åû§":´Ô¿èþ8
,Ñ¿ïÿv¥NAGNbcu?ïÚ2æÝ?š¡f§åc?‹S[ðâBå?"ڐd#±"?[³JAX?ˆ·[
Aì?æqœû×Y÷?Ëè{²†ƒ?µË/ò>ª?²3©ÃÈe?Ë«&x©xÏ?ƸSŎ?ëøîÏèn?¦9ê	-,1?±Ç•n?Žœ¾Ñ²F?¬âúÄSlê?–RYË¿>?èg­"?«7JÖ¡	?µC×Üè|??£{"S?ÿ_±–eˆ?¦3PЭ ?ï'Ä:N|Ý?ˆù6?mƒ?zû­úà?PքvØ?|Z'&×"›?wò›;ÐÓ§?ì¿z&6Ën?ºØ¹·h®â?Ÿz'ÿ\Ó&?¡£F
Ž>ì?²%ŠàcE?³/i*?Û?î8|÷ބ–?"¬üì²î?¡©îcɟ?ñ£¨Ô&?•ž!/þßê?€)XMzÛ^?í¡¥€œad?'ÕÓdI?˜î؝~¨?†œÍ¨*[?©n;ìÇm?uahì ÒAGN3FGL J2111.4+4605@Vy?ò^W¿÷v•âHŠÀ7ÙôŸy­kÀ:ÔàáVǍ@›}¸èi`@©€`7£@EÓ¿b:¿Ôqeóп۔Îs•ùÒ¿ä$Ä
'f¿éÖéë¸í"PSRPSR?™ž³x¬©?™© j¼D?ê@F/þå?Ć€si?Ä¡‹Ðî×?ÂS:Ò0[_?@Ô	•åÿ@?^6¢›LTs?æ!õ`Ï_?¼õ£ÒL¾?Ó³«¾Š>Þ?¼ò'ë§?Ë)—Öp¬?±"9uéýd?߅;[ÔDÄ?»VSìÇí?Òåø¹ æ?¶P0>÷¸?ž¸spÝZ0?Žƒ[oO_?êRÉ	/ò?­9R{Փ?ÂÝÍl82?©}™oéw?œ†µ·˜Œ?¢PfI
£?ë7	ûñr?Àøîôiô»?¿&¯C
R?½Ûÿ½?]Þâ…e
?sÔB?æÂ
ÜXþ?µ`ËôMI?Ò^"{?µG²¹S²Õ?Ñ'ô;¦Ÿ?²μ†Æ"?àqԘ{À?µì¯K¹ƒ?ÌÖÅ&ÃÂ?±(+'ÂúU?ª9[§d–?¥Žy½Ì£?ëˆ^o?¢cJ:&f?ºBґ̊v?›¹|4š@§PSR3FGL J2112.7+0819@MZqÀ6¼UÀ:OoŸËÀ9‰˜ð&n)À;b8¤Œ;ã¿Á"^¡\@r¸¥š"?ü昛ü ?݋ë¨|'Õ¿ì®w/?j?Å¡(†Sc!¿Ýæ×½
3'AGNbcu?ïð²a*"?VËp¶1d?$ñ_A? ¿Ë±Ené?\ÚUÕT?VA½wŠÊ ?ïmÓ?'¡Û?	¢­Æ®?qŘ!Ë|?}^?u;¹e?‹¨dìIf?ˆz5ìšY?
Æ£N?Ïê¨CÅA?‡›ë4j5–?x*º–!ë'?ŸȲåg?Ž]ƒª@?ím÷T_Ô?¨ÂÑU°|-?@Ðؼ‡Ý)?K2ùŸ²fS?³râ÷?¨Áhs9'$?ïøùÊ?D&CI8ñ?$&}¹-y†? ëe4Q\9?J¶{Sô€Æ?BJÉz ?ïÎ¥µ0ÎÕ?q[oŸÅŒ¢?YÖ^'¥¾$?S¾3yû~Ç?r7ãëe×?m5̋ûs™?ïh‡!‹¯»?}ïé,·í?{
;~l}¾?nyƒ­~½È?ˆYߕ g?yˆ'8]£L?ïi&"מ?q‰ëà¾?Eù!Ë©?=¤æAN''?',²I*Ÿ?€Åõ7DAGN3FGL J2114.7+3130@S¢åx•À'Äi¿·:"À9ÿôU§ÒBÀ;† Ô÷=º¿úÂc·àV—@Er•É«Z@ʺŸÎ'ô¿á?+¡Ä`m¿íñw³Y¢ø?Ù"V³¸¿ì¸ö´&ãšAGNbcu?îhvQÿ?¥{™›?Ý{,vß?"aZŸ–?¢8`Úæ_? §ª˜<­?ïV#?'"ÕNé?~'Õn'Ä?‡¦WJÈ?–Y_ÚÀ‡B?˜QúÐi…?ê0pZÛî©?§˜¯ë"Ø?´¡é›æ?›tÕ_°y6?¹Ú" 2ûU? Åôޒ?íû;¸Æc/?°•.ÕÏ?C©pèä)Ï?dµ«Ñ00?¯ýž³¬6Í?°€a¯ï»?îà`ŸÛ†?°çSÊx Ý?}}J%a'?neUE´ò?œ»T—kré?°Bœ‹%2?錄¸šÄE?‡}7Ô¦·š?jc*ʇ?qPR*Å&?€Iù
ÔØ}?€Œö@¤Ž?ì¶æHô»? ÑI†¢?1?¬!·x¼O2?—m=:áû?¨}êDÉ?"Эï‰T?ï†æ>
ï?‹7"NúQ$?*	8Á"Z?6-budó?ÞK£%|?Šç©ûo*8AGN3FGL J2114.9+5448@WÁûbâ@'ßÕ=4À9Á¸øÚqÑÀ;ÉÜCbU`?ø½üë"£C@·\^¥§Å¿ùÄ™€í¿ÞYÀw÷)忲o¶*ÁA¿Øђ©æBë¿îiYÙÌJØPSRpsr?ä£îGN{Â?Ú³«ÂÕÁØ?ÕÌå*'?ٞÔu§L?šµvMz­?±ˆê@m[ã?º5-ÎOô?Ê¢¬¾?à¾Ûқ6?ÓCžF!ß?×ôüèY¬U?ÑØ)¢:Ó?Ê?ìÝÁð?°F\q9y?ä^©t^?´+b«1??ÄFÚmQð–?¬j8H"ñ?Ú÷f³8~?ÒMÞ<-O;?Òû!¬Ö•×?ÑsúzВ?Ò
wŸPì?ÒêoÜ(Í?æz«´="º?Úxÿ½‡W?Ñ'Úõ>ö?Øx=2)a½?ž,èGOëh?±Çê¥OÛ5?ÎC
u"Z¸?ь5Vè³Í?àp/¤µ?҇èIÞxú?ݘæ&¡;?È{s€w¬?ÖÚZ·(?·¿û˜$??à–Î)÷©?·Áí7àÉ?¿æý-Ef?§Îu!ãÄ?Ýހ®¼š?ÍS'šMÊ?×éÏû3<?Êõ¾Ñ•'?Äo^®GaÐ?ɅkˆÓèdMIXED3FGL J2115.4+2933@S'"Àh¡À*™egÊÀ8ÛN?(3üÀ;lw—|?áNø>ѳ"@ʱ…¶Ÿ@û
_d¦¿å•´|ôÈ>¿çæb3Ò¿àÔ¡Vì¿Ü]™j#AGNfsrq?ïèx qþ?e%Uçkö?Bƒ¤~£\?=®.Inܨ?bæv¤q˜Ú?c·d<ÆR?îû´k?©rÇQE"u?"v?À;ò-?Šó쀯-y?M¦§ˆ?¥•N€H?î˜èŽõ%Ü?'ô§€cÇã?‹ÎPöáŸø?z¼$=¶ì©?žûÅ¢zØ}?»ä¶è#?í>¼ÇØ,Ž?¢$¾6˜(¼?š•&Ÿ$i?}Xs]:†?³ÖÇj·?¡=†Ä
ù‡?ïö"úMŽ~?S[òÀŒ'œ?6.¹m-iO?2Xà©gÓ?J"º£8‹`?Pÿ¾Ü0,m?ïˆi¶R?"K_
"æ?pù¯¨ª|?tM÷üå¯?…ו£vÚU?Ž§(n T?ZŽI?té³Óx­Ò?u[ÌXÚsì?gŒÐ¥Ü?€åƒ(É4Ø?n-$ñé÷?ïJÁæÈ?ƒ;¹>ýx0?rä|ï"bÛ?]¨4Ð3å?'^ÿF?'±Òp[ÐAGN3FGL J2116.1+3339@Sóˆ` ÒÀ%K@¡À7ôò3Ž£À:Öøp¿…¼?êíª2‰b@AVóרž?þ"ëßâ~:¿Ù@Müì¿à‡Ùí`"ê¿Õßy¬X&÷¿àŸA=%êAGNbll?ïì<\ZQŽ?^Ûò¬yÌ?3M£©_Š?6rpA?aYîôÂò?[ßUĺP?ïDåã@¤?˜§ÁCsf?tˆ_U=-º?u84Jî?'KËo$‡?•EЙµô?I!˜?™Ù
	ï;?†]¹"lÑ=?~¸Ý?­]O?¡÷‡‡.™,?–a'P«èF?î®
^ ×?• 
"ºÐ¦?Nùœ^ÙO?WÔ/	µbÜ?¤£s¢¡?•S6ّôb?ïõü‰±wº?Jñ0Ž'áç?)Â4þ)Î?#'n5h?PÎ¥êà´
?HTtÈÿØ?ïº$ß»ðd?}"¤#H?a'hýv?_‡¤~Ãã?zYÛחW%?w¨ÔLÉ?ïIÍøW%g?‰0D\5ä?€•¤ìWÝ?w¡¢ÿp?ìBŠžg?"ÃÒ«¢õ?ïÙ{ ¤?r¦Æ¦?Mø¸ó{)f?BOúW·.z?†ª–(ñ?qê†\€'AGN3FGL J2118.0-3241@(üT@Éô«ÀEó; g~"À:BÌ}À:æÈ~‰rÛ?ۊÒðÄ@
CùÂ#P'@|#ꬿè­Xíú;g¿è`"·"Ò¿àƒŠÚË#f¿Ùq·z!¦AGNbcu?íþ,Á)?¹Z|ÿ(@p?cFiß(WU?hðÎéÅ?·=Ä¿Ì®ü?¹:ã‹2×?ïtËöÒÉ?K57¹7–?kJ•1Kmº?qð0	I31?Œ,çÃö?‰*Õh=0V?ç˜Æ,l?³½%®Èý?°FցË? À甸Ú?Ëmy{ÓW?±+F;ü?ç	ðÕÑ¿?Ã}~ÛÓ%?u;ù€·ý?VCaá=?Ñ~ü7§Þ?ÃA'éÉ?î]®ºp²?³ØYŸâG?NºÌ?[³ä$Ø~"?§<¸0ø4?³µùg›«Ô?ïÑHãQQ4?s&ñð¦d?UZƒjq?TK»³Öw?r·Éº±ˆ?oÛU '?ìyq¹‰?¨rØÐê'?Ÿ©}áa?'NZ¾Øçd?·¤ìò9Ì]?¥N :âBð?ëó	~r»x?¯î>*•ÒP?¸ãâl?x¬[?¾vÓ#±""?¯t§?4>AGN3FGL J2118.4+0013@Iû
ÿ±À@Œ@ÃÀ:Œ"\BööÀ;ÓáYKË°¿âM4CÝ@
Ž°?ÿ_@wÏ?4…¿è&Ÿ«Ÿ¿ØÀúýÈÔV¿Íô÷×E)]AGNfsrq?ïú¾zN¥ª?<7ãþ=Ï?KhþY"o?­0_yNT?B¼ª@C˜<?:¨2!ŽÅ†?ïŒ@i–`n?‹¹ÉNã ?gü¬ÊŠ
œ?{U"H'=ó?†ðºr5?ƒÔœÍr8~?ï5ϛÅT?'w¦¼*/Ú?
dFƒ?gÎå§ùQ?''³r4…+?-֎(?ïmKv÷?‰÷ð"M˜ö?"ˬ‡]'?'³
ü,v?'15½ßÇ?‰ãP€î‡?ïýõÚse?+ZCt$?«ÅJ"æ€?ì<ƒáX?4"×´•=I?(½Œtîm?ïÝaŸN±¶?lpbÅ?Qdâó̶?PT4^ns?j®qNÃ#?fE}†À-j?øA£A?pöÕï<6³?sŸHEñ&J?X9"?€Ä–¡?k'yNõU]?ïèÝhj;w?`_Øø"î?ü·x–s?Sԍ9¶?fš±¶ÆÃ?`Gò.ôp¾AGN3FGL J2119.2-3313@'›ÙÀÑÀFê jšÀ9ëãïÿüÀ:ê ;ꊿè6+±<V%@ñ0¯J@ÐÀ¤ ^?îtXûLo£¿Ø	2åk»K¿ì1Vë…ZÙ¿Òàò¹pyAGNbcu?ë!YÛ­T%?ÂpÐ{ò®x? ¬<õ^#?¨ÌœDQ,?¾Ÿ'"ö–Â?¿÷*2Gi»?ºÁ?‹Ï³/´ý?hóÞ¥bˆµ?rß"…~?‰¾'4·½}?‡(Ï<ÃÔ?ç=^$è1?³s!'?¶:+ûÕz¦?¡ô£¬ ?Ç]ˆê?°ã%Ç\?é´ÒÜ S?¼qÖz(BÈ?gá)»©§?o·ªªÑ¸ä?ÈÍ.QL"î?¼Uã'ü?í|æÍ?ÁÎ5˜Zö?€¨U|Ü?'Ò0sl1¢?µR=û?ÁKÚ¶'Ä[?ïÒùê¿9?q¢~Âk0Ž?Tw‰HCˆ¼?RcdÄÉÊÄ?qe(·Mñe?nWF¨¥äø?ëèÝר?¥Û¼ÒúPx?¦ò7å·?•ˆŽÑ¶ä?µ?õÁì&¸?¢¬ë:^P?í³Üp%Nf? ·fÈp?Eû ûˆŒ?@a\º3Ï?²6à‰9œ{? ¨Ô
øóAGN3FGL J2121.0+1901@QPàÑnÀ5A/¨;ôÀ8iÎÜq…~À;FŸù/+g?îrIƒ#,ø@J»Þ'òá@DŸWž¢¿à‡àUÆ¿ã0ÅDÿàã'æ&]¿è¹;–
)AGNfsrq?î(u;ã¨S?§Kb—š~?£‹×D;?¡ã…Tuõ'?"¶@Õnm,?'XÍúÞÓÁ?äŽk
ü(@?ÉlºÄÈ­•?È'ò¥i?Àü`-'4u?Ÿ+Õñ¹–?Á9»Ã:&í?ë;õDÔà?©™çwf÷'?°Aí"ÊU?š«õj9Š?µ†>iý\¨?¢1,º÷vê?ân²Ø&i™?¶\z‹S´?Äj'ƒË|?°¨Ì‰eVâ?ÐíQÍnÄ?³Õ…klé?ï_	3õØ?dù Íˆ?Šh²^6?‰{k8æ®ÿ?{ªR.Û¿?u׈Ջ"?éo£¼æ®S?ÁF3;ÒÐ-?¼‡ác#?³ËŽ[PrY?·û`4eeÊ?´È-£w?î(5+ŽÁ?š(tÝ/m?›jZìԌÜ?µÆyw?ŸŽÿ£ÿ?'S1ñ¸Á1?é—Lß_?¥LêõµW?ºÇô¬j?Ójê'W?¸±†J\p? 3P>¸¡AGN3FGL J2123.6+0533@Lüa_–hÀ> KŸ:ÃJÀ9í.÷<À;®á?J˜«?ÐU5åGËy@H°Vï¦@`_ÂWÿ¿¸
PíПã¿åk\¨U&׿âGÁÌ#ë©¿â<I}³›4AGNfsrq?ïð9í9î?W=Íyp³_?/!‰Žì!?&%ûȍˆ?[¨Ï(/¿?V1!!ñ?ïJÄðh?–p吞ò?s ¬RÄÌ
?q_*ýÄ?'¿6Üìòµ?"êßl¡9?îÛGŽ‰ñ?ŽâûQ3h?‰Ö܍b"C?xBW±´?—°èÄ
ÜC?‡äq ?îî-çç'?–aà‰†ë±?v™"B¾Å9?më̸ô†?¬ÝìœÛIf?•ÏY%'…??ïøÁ–Òƒµ?Cð^¬›št?%Eùé€3Œ?åH>MÎ;?G¨%æçL?B5d"É,ï?ナœa ?}iÛª¤ó"?`oi"ÿà?XµDpIv?xºú}Bƒ?z	ïœua?á҇;?z=FTö˜ø?y¿3°Q?kAâeŸÈÜ?€Ïf/ãá$?sçùUñ>?ï‹ÿù'§B?uÕxV?fb|Ámá?R™0ïˆLä?‡gb®®¦2?sÏõ¢Œ8AGN3FGL J2124.7-3358@%ß# îøqÀF¹ÿÅGÀ7õˎß+À;MÀ‡D,€@ªaèÓ>@Käÿ¬ä?õƒ…UE¿¨¨ƒþc¿ÒPòÌ:֖¿ä¨‰{¿ï"å™ç+PSRPSR?p‡_ñ‡`??yýæQƒ'b?ï5_²1ó?¨Âµ».?•21Å8ȍ?§V
cüåÕ?{Í
~‰˜ÿ?ªÜߧ`zÁ?ëÀq»Fy?Ҋ¯yˆ`?ÀÓu?Â8NÆ6°–?•F+žÄo¿?‹róñÌ?ëä\!­¾ƒ?°ÿê›?»‹"*Ês?®¥ëbiJª?nK l^²?fe2ÛÞ±P?ïÆÚ;î?'
¾°V?™"õ>«t?ñþ·4òì?bÇJÒð&?pQF2+.?î²1½´£X?½Ñ·ïè?£°os%Gª?¼ÝÉß²'Ÿ?"HXß?@2?—1‡Bœ5?ìOZ¿û?Àú·tS—Š?½<{ö	uä?¿_	Ìm½"?¡Â¾®n@?™"ŽJ[ÿ?ë¬ wü?¯ªâÏR?¹½ò ¶¢?¬Cš_lk?}翼ö?kºèØËÐz?ï+1ûÙ?ˆ]};?"%OPèSP?…Tx—WÂPSR3FGL J2126.5-4605@všßµÝÀFÒf€g™lÀ8Fo?Rü&À;….0Dk?ñÌs)˜U@nšúíœ@¯àÄ¿âúz§]sñ¿çžâ¶:††¿çê^¹ÚèÕ¿ëøSçïÏAGNFSRQ?ïôÎCW?P€úq	ÕY?I%Ÿß5Íã?HÚý¾‡´ë?F›&r{FQ?@s)´Æ?ïˆÖJò9?†%ÿ)Q™6?g^—C_È?hN
nªÂá?ˆ7òÆ­Ë?'G²·ò{?î«Ú?ëÂ?'t
—8Š?—'Õ""?ˆèÉFtGi?'ñôäð?ƒ¸weTw?ïÌ<Kµ¶?{•ŠÜÀ—?A‡3"íu?HüÐÊà?w°ó¹†Û?züýÅ|Ç2?ïöæx'Ù~?R'ª"w™?G9zSdø?KކíXèÉ?:©Èá´÷J?7b樕 ?ïÖôÑ×+S?mç!œ8ن?T@ôòǼy?RŽ2›6?n곚Ó&Â?fÓè­MŠˆ?ï+çÀÕ.?ƒõª<U?åúœóÿ?{>ÑÓ±?… *Päß?r×ì¬	_…?ï÷$é]@?Xv¬¸7òé?,å]E¦y×?-mÇ|ê¨?L3O"ž?WH|ûdAGN3FGL J2126.5-3926@ú'À9@"ÀGÅ 0!0À:^
ÒPšÀ;ç;¥È|?Ýv­©ÏzZ@
eWСm£@ŸÔà—"ì?ëíÏ¥³òû¿á
§ù®­'¿ß¡¶{%Ò¿ïÿuQCr#AGNbcu?ìä¡Ú}0û?·Ç$‡Ã?­0vðkEE?°"•N¶ee?¤…kdR?¬˜¡ïJóf?å±Ü¡ß–Ý?ÅÖs–Çúw?ÂæUõU9?¾l£†QY?ÆR7ƒ,£U?¸ì	(ø»¡?èdç?°	¯Ð>|?ÁBçh%ûŠ?§§–í£Ï+?¼—Ÿ¬Ðz?§®;0:ò?ãÙí,úÆ?¿ðuO–?ÉЅ>é?»ûŒ†iCÄ?ÇzÆÖÏÁ?²{'§\ÜÂ?íà1À0K?´3cG·Ÿu?£`ñÿ7/?«Þ}Dìq—?7åó¯ý™?©ä)'Ó?놃n×E™?¹aöqw@È?²¥\#û'?°êØ ?±&ˆc%8?ªÛýMef÷?êÉi"?ªâGø?¼éûötÕ¯?¥E‰_§?²G»Ë¢¾?¡4æœ~‰?ëˋB­"e?¤",(Šµ<?³w	µe?žá®±-ßâ?¬Y8·s͗?™úÍr+oAGN3FGL J2127.7+3612@T֟ŸØwüÀ%%ó_ÍTÀ9\M}À;DÈ6eÛ?㛽®CA@¼¿ºÀ…Â?þb±Èd¿Úè—-®¿áDâŒôçë¿Ô©fK
šr¿Þ"%öx†"AGNbll?ïGÆ¿±J)?ŽEµ‰˪?r¢@ìã"?gݍáÿ?'g?v¯×?‹äoÅy‹ ?ì‡N›÷ö?Á#±¢œD?š‰›vràä?ŸÞ-§•÷?¹1^­"•?¼ó
Á¿?íÇ?1n7?—@8^©@?›~«*z"?ˆ6nnEù?¥Ì·W‰m–?*_«àcÆ?é5ß­F—?¤Í8?"²˜"uäì?ŽòÌÕuÍ?Ç(ÕpN5‡?£êÃ#,Š?ï¯#"_³?uÇÀÁÏ4Z?aޒwß[*?Wg3Cbü?.ær½C?r ä&k1?îkXÄùTü?®ÁA*!#­?ˆàra•rù?ùsÐî?£W½!{?§¡N oŽ?ïnèÀô'?†ŒKKÐ/?‹NcŊ(Ü?zXÑä²É?Šñd˜Ä?{y7öÒ´â?í ºÏcî?Œ¨äH%l?'"¤‡÷?C?y;õ";
…?­*Èf†~?ˆV÷ãšÒPAGN3FGL J2129.6-0427@Hu9ÿÖ•ÀBsÇä¡ÖÀ9G¢[	;À;"ËÚ^†?ôß»6¢S|@dëÑëþ@½' Pˆ¿Ø]:vQ¿â©'…UêÿçY¤4ŽcA¿ìŽËj!0ýPSRPSR?Ûà(µ¼öý?È9SJw>ó?à‹ggËÉË?Él½ÐR	Ú?¨HCÏXZo?£X±T×?䲏Zæ?¦ï"39z?ÅÕ?ù6°?½JîØv?Ê "]¸?º-@Àd‰—?Ú$҆¹ÜÊ?¼;:h±š?ß$8@Z°r?ºûÊs"®Î?ºÛÔã­Ë? é‡õU¢·?Þô€µÇø}?­ïΞv2?Պšù*4?ª:ý6)»?ÇȤk|?¬X¦mê¨?䩨tAµ?ŹÌ:÷D?Ö‰üºó~?Ŗ·(Ã+?›+%ȑ?'V'ŠûŸˆ?éa¼­'AX?·°aslÇ?¼–Pìâ¹?±­Q¸ÀŒ‰?¸[Êz8à"?¨×ÐHÇ*?æJ‹âi}?²¼ÒêlF¯?Ïï¹v…?°—0€ŠÛº?«›0øV?•­'7Må?珳°W\n?¡V4'?ɾ¸	ú³C?›ž‡0äy?°òiO¶?"ýúÇOíüMIXED3FGL J2130.8-2745@3ÿV_ˆ%ÔÀFéaÀxiÀ9àwŸsÎ.À;¾:bÒ]?ðÍB"xm@
£*ƒ6UÒ?û-_ÿÄñ·?ï:ÀÎÅS?íãqàÃr¿Ö‰í›	Â]¿áoxæñ'AGNbll?îá—pä2‰?¡‹Ñ¦m•ï?{vZ?0«?Ž»wK!L½?
4P-ƒ¶?›ÊԆæÐ?癄®Ùzc?Ƈ"ã–+À?½×aêðh?¼"AŒx…?Á'~ÜÄ?»¸iøl8?ë~¯/$?§Œ~8Ré?­	 £F?—Эï‰T?´ÿ‰°¿ç;?¢¦Õ-£º?áFÃ]?ÄǟàÊI?֖vãó@?ń>†¬	¼?½Å–UJ?¶r
ít$O?ïNK¼ZÓz?–À'?¥?u/AŽô…?yDW»°G??êÁb2¢?"w¦--?ì>Ú$	…Ì?»…V'D ý?­K:àØp»?±DhB‰'?®Ç"ßk…?°yÓP€"<?îTw¦±?™
ÿ47›÷?žØ¯…Ék	?€À`¬ó?üÁˆÖ:Ð?BÁÝ·¿?é.¨"?²
+°x|?ĵw}‡a«?®TºÜ#EÄ?¬Ù …@"-?¢ë¬V¢³{AGN3FGL J2131.5-0915@Eòp_äl&ÀCÕQßƤ•À9^YûIÀ;…¸¿Þ¨?Ø´öp£ðÏ@߂ÃiKÉ@1ÿ¦™¿ÜVÝaÅlÜ¿ç€À¶F¬¿ÛOt2$¿ÆW†àÀ†AGNbll?ïì{Қ}U?[ЧÊJ@µ?Dܗ>"y?F­Å°õ)s?\šöL¯?UsL]èœÄ?ïrõMýí_?ŒÞü*ˆj?i]¯<Qí™?rMUþ9[?Œë@°hJê?ˆ¦y÷žÏ½?îӘVߛî?Š'"n_Ð?ˆY­Èf?vO½«eU?™`hЗë@?"(Xÿf?î5ǵ`Êp?›§
žÄ¾Æ?YÏ$Îô¡?bgü…x'¤?«Õ'X´V?›;I%dÌ?ïøµ»ô?AL†t°ws?4ݓ.žŒ?.væ8bK?Eôº¼÷c?:_ÿ+7þ´?ïÐ𶔄º?s,ãX?ŠA?Uòuž×·Þ?R2Œìé<?rL§ÜÔ?p$°·¹x?ï€I±¤Ó4?s8ëñ5¥ê?yŽú6@ô‡?e,êÖå_Ú?ƒ&{ª¸Ö?lÀqÿ/£A?ïavUo?w£p炈l?R£31¨7?K£W•t?†S;úµD?vÜL™AGN3FGL J2131.8-2516@7‹yœÝòÀF½aßîèÀ:C(ǀÀ;×>â"Þo¿÷Æ<lí¿@´Ô©˜@ÿÿ&§¿à¤\—ÊP`¿Ú§Û%Õý¿â"Ò«Å&v¿Ü.ÛHP7AGNbll?ïâüž˜ÿ7?bþ¶·‰/?/€À£á0c?#ªÁùaZ?kU'k:C?b‰Àÿ&JÉ?ïƒE¸Ø	}?…ѧ·pmq?dA։AS?e©Ð	0%?ŠÆCò?'æi²rlÓ?îšg^LÖ6?Œ åvéu¸?Žß[¦·?|8ÐÒ#!?¦K͖Ò?"LÙ~V.?ïi±ÞΛÉ?ƒ·GÂÈÐ1?1K7TÂ?3†Á9Hc_?'…J÷ü?ƒnM¸?ïó´°ÔÒ2?S†÷l'ÛV? tH‹/?0íÿ÷"à?V"ªöoÿ³?S"ê,~?ïÚxåwœ!?jð€?Qã|$]iR?P˜§¿¹Ì?l•\£±?e:ê0¹?ïpBՊ?rÚ6džÕ?|"0·nõä?fÕPEé÷\?…Þ2;@¼Á?j0¼+,
+?ïáçöÐã?\—È	¡Åß?
p£ðYÝ?	…Ø¡B°?m®G |¯?\h¦»ÍÂ\AGN3FGL J2132.4-5420@u]8À>-ÀFqEÄÁfÀ9Gíf H
À;·¢šÊB¿ë¾É e@d¥‰çÊÕ@X`"?h¿åÊv''²¿é´ìӟÇ(¿á†1/D^¿ëˆÎé¿7AGNbcu?ïùk§Û.?FÛ3z>Æ?$Ÿ%oãŠ?#©sÙ;?E+ç³OêÆ?D¡šæ_6?v:;]?ŠùÃÿ2u?g×E!j?{°:Ã$Ä?ˆ#8GÖ??Ê•LœR"?ï
vNð?"©Ÿ[?‰–»ØX¨*?wH•/ӈx?'ò3Iê•ò?{±2˜P¿Æ?ïšyoqkÂ?ƒ0Qmç'W?5½¾¹ÒØ?:?S]˜?ˆ³¶:	Q?'àœ"åý?ïüb40;æ?4fRñ¿ðœ?#Ù©Ap­+? Awä÷1ç?3ˆR®ø˜?0‰é°gç?ïÖwSÚ¯?oÂIì~2&?S—FŽ«?Rç³ü›ðU?p`¤‹Å?ivBW¸€"?ï{Ðè}­?t"Ô'˜ht?J
`'??oۇ'Œ˜ù?ƒÚø'ï?f7	qºÍ²?ïíҙŽ'?`óV$Ø?ÔQNc?GåßB~P?a¬¨-Õc?`wÿ÷ä«ûAGN3FGL J2133.3+2533@Sy?ò^WÀ2ñ1Àll:À:IÑqw<À;¥É¤úì¿ìþgƒ¿4*@
Ÿ3«S*t@çU ›¿ìxÛ¢S¿×gb!sK¿Óþ;ĕ¾¿ãÞ
ùÇñ`AGNbcu?ïëÃoMb+?`E½Â¢`??3X4ïmÎ?/®o*"¬þ?aщìC²Í?^@K'Ú˜?ïLÓЪ°?'ÔS%'J¼?tYêñ¿º.?võòÆÞT?'WŠÁ¿œp?D¹ÒÐñ?NôsŸ?Šñ©ºžØæ?‰tð43?tçF¤jà?œ¥²ïx?…}RÙD>?ïÇ]}_?Œ›ž5órw?Jr%j?Dï:¹É4ì?Ÿô(Õbþ?ŒZÄ4Z?ï÷ÊvRº?JŠùüõ¾µ?#dk*HmR?oð"ʺ®?Oºkä´Q?H¬øDp?ïÅýæY7?v'ãýoqÈ?[(YIÐ?T¢°ç'?v:ÂÐrêE?sàŠ"éóÿ?ïuð|q?qiÇÖV+
?z'o:~H?`# n˜?…ŒLR^´¦?ibL€€%Ò?ïÃZ}yþI?f#Õð©u+?8¼?C£?*º¾'Òy*?|Ño<"…Ø?eµÞ'RÓAGN3FGL J2133.8+6648@ZLhß½jY@&5Á'ì¯À8öüšòÀ;Fçž	jãÀ»zgODŒ@·5Œ©Ç@ŸMÀ¨&O¿çv\{è¿åŠÝì&PÄ¿ÅõJç¦9¿Þu&HÐ9¥AGNbcu?ïúÜäa$?C0[C_L?¸ºl[§?Bí
Îù?AØÈÛdÀ«?AÞå.Du%?îûº;òí?­CCé‡ð?oÍ–Jé?qù[ǘÝ?œ¦¢AÝ?¬®Aânj¦?îî"sJ?'ê±Äp£?O=á%4?r"á‡_&v?™†Ème¶?…†¥¿B?ï×o㒶ü?q.öhÌ¥>Ì`1ï{6>âá['v°?tD'6ã®F?q-,ªù(y?ïýÏä"N"?0°7ƒ¢ü?õ1/ß³?·LÓW ?)!/×Åö?-U2[	?d'õðæ?ÿv ¾É?ZZŽtØ?^¯E}f?z¶ÕDŸ ?‹Šҁ?ïœ%Õ҄ó?tßùlîa?rLì°Ø{ˆ?bØÔ¾Åå]? (Wv¯@?n"öˆd?ïö'?'C^?N•ÎT1y>¦……¯ÊÛ>¶LFW¦XF?Rø°3n¬X?N"ÕéIAGN3FGL J2134.1-0152@J3lÿݛQÀB>Ÿ¾vÉÀ9ÂzcÀ;‰Ê)"]È?êåúr¹9@_Ə@¨õ (š¿Ûk–/§¿åB¿©^ð¿á*èàÃh¿éžäq%©AGNbll?ïô@e•¤?N:(ҏ£??Î|‡€®²?>0»ì9›é?O*ɗ5)?F-ÌíŽh?ïi?W6{E?Š½œº'²
?lcl|_?mâÉ ¸aÒ?Ž—bRr£?‡Mùß´ÃÝ? ßUˆ?"ÃóX~|?˜¾
á1="?$T‡¼ƒq?—A›ßß?…ÝO;l?ï[ªZÜð[?Š'èÇÌ?^º	%?ZìExø?'ŸÐj¾?‰1ŒÔŠ"?ïúRÕÌ??¼ù†(1?5)Q	?0³¼²Ë?8?ÿ\9À?2ø1æx?ïÍKæïsý?rš®—'"?Yog¼[Ì>?VSŒû–°Ñ?rþ2'Ÿê‰?mÕ(¯'TP?ïiñ¯@†?Ê¢Â4ˆ?ƒ3Á!?º.?utî©h\?'OÓè3?s6rM'i€?ïÙ-%R?i˃'dÓ?RÓ²¢²¥?E¼ËæÌÚ?miQˆæ?g—JMÅÊiAGN3FGL J2135.3-5008@u·©³únÀG1Kÿ²Ó'À9&*·c®üÀ;ti;'§?å¦Qs˜±›@/Á™gð@Â7r@º¿â]Pì4Nſ磷쯯õ¿æ
fyG¿î97²ÚïaAGNfsrq?ïÉú[Œ?w®£@µE}?o‰îm£ø?p­T0¯?gnö±æU)?gۊµe$
?í3Ûñû'?¬"ØxnÕ
?œb*´
Ø?–Ns'8?°Õ¹ÖŸ
Q?¦Y•Eí?¥Á×?šC'ÇŠ	?£gA®{G?"|ý¼	Ú??˜^Ëp	?ˆ…ôj-lá?ç΋OBú?¬`Aâ#K?´ŒŸJ;?ž=+ÑâWÆ?ÆÒs)î;?©§¹8"'?ïÐ='±R|?s ÌÚ`ú?p!†t»=?nd½ H?^ÿ–ûèïÇ?Yíñ95K?îØïl¬H?–äJ×dŒd?Ší7³†¼?'KµkÍOŸ?—kÕ|r?"iddÜã?ï
ÅèúLY?‡"¹©´Ž?"ÃGIr?'7°g†¸?…Ç÷@Œäµ?s!ædºs?í&§€{Õ'?•kڶȾ?¢ŒzsÏàœ?†£-ÛÊ/}?«	
‡âhê?'—|Û^:<AGN3FGL J2139.4-4235@vdڀIf{ÀH)οìºÀ8àÇU"‡À:ýÂÅ+?öùŠ¨ex@ðÀêÁTt?þ.` ©®:¿ÚÚ$¿à‰ñ]]%¿âª-qI¼¿å¹·©AGNbll?ïéá™ý0‡?d[+•1?3g"qÂéë?1å¨÷*?c±s•üé?cúoþ?ïm/2?Ö?'TàÊ3)?qÓ²,( 1?Ú'­º?‹ÊZN!˜x?‡q­«È'?îgoj(?š«s՝}j?'´ôqlÚ?ŠªHâs²g? ®Ç®Hàì?"èœôÞ\ï?îï×$$ß?¡À¡sÂ?a?uñ;‹Ë?yjnÉ
oK?«Âßj⋡?¡E)¾‹¦?ïøW]<¤ª?P:ƒÕŸhæ?$ŽÍŽ˜? ËcÎot?I¦Õ¨yÂ?OšzÞ:?ïƱ®ýó¥?uâ/ƒOÿ?]õߝ6j¡?YáêÕÇy?u)°¶•J¤?q~r=‹'?ï&š*…‡
?‰öµÖ'A?ˆÐÆÆ<S²?€~2w®Ý®?ˆ®''±¼?'"ÿ,E+L?ïa-5('?"'äøòØk?r‡åöÆ?dI þ¥Ôe?Žp¿ó¯ìk?ƒs0OYS¶AGN3FGL J2140.0+4715@W(üà%o%À-J?¿2°À8~&vŒNWÀ;9ÕÓ܋‡@ÆèVÁ@
b)Üó5—?÷òˆæüy?ƒMc¤ÙØh¿ßæ碈x¿éÀ9ÖæV6¿ïÿߓpW"PSRPSR?l\±Mi¼?vϹmÌŗ?ޙSÿûù?Ô3'ï6?à–ùµW÷?Ô;G¹Òõ?+Ѐ$~?@±1ÈÙð€?ë܆Ʈ$Á?·I¼­ŸÿÈ?À‡¥FÇ?·?WÌ`9}?œv!´™ã?µ?^Üü'?ê>ªÀø?±âhçáUd?ÃxÑöH$?°ü.Vƒ%?q±`ìJµ?guÍÜG6F?îÅÄgà?˜!n·./1?¡'ü?q©?–؝‡Ý&?]ˆ"ü‹?lÁk™x?ބ÷èü¥¥?Ö[1:EÝ?à®ø…¯¤??Ö4C˜Iý?TxT‰öã?†ì­(Fäú?ë´í£î†?±zGóÕ?Á~T³z?±nwÃ5=\?¦ڋV~Ë?˜\êƒð?ê]_þy(?¬äyê6F?Á	[A³î?©ô'dÇöf?ˆGS$
?sïó|;Ë??î"ë¢Ùfí?'ÛÉMÍx? ¿3ùU¸?Joì GvMIXED3FGL J2141.6-6412@t‰¢ß"xîÀE!'	±À8úÙ*© öÀ;¦þÍÐØË?ñ€=û8E@"ž­Õ'@ö?[4¯¿âuöÉk¿ço7HŸ3À¿ç>‹Q¾tÖ¿ïûdÒÁAGNbcu?ïéo¡3Òü?Zu§Š:±x?U¼Û"³?O‡"DB°?Xm€d~?QýºÅ'*Ö?ï\CK%»?Ê´Âà|ç?o,­FP?q"ÎÔìXg?˜ðÄC~?ŒªNÑ'+?î[¨VîÈ?"¦+
`OM?³Ýï];2?Šóÿó'?–×1'Ü?ˆrH}åb?ï"U c?‹evè™ÐÚ?i®ýaõ¨`?h'ÆÀ/Ý?ˆ~ÜÝn¹$?‰r^Ú:zy?ïò(±¤þ'?Vž\'òX?QM'§±c&?Sø[ä4~?DÂi›Þn?;Ÿ¿ës!?ïÃ;[JA?vy6`mr?_âÔíC?]:ÝjäƒW?viÎ5d´2?pÏkeIé?îÝp~Öä?ˆLÚ-Í2?—
w,{@æ?;ä%¼¤¢?Š'¢™?wæ.áÛK?ïã½?CÀR?jq¸ÖSí?Tä¸Ä´§Ë?N.Z€Þóz?aÐdg£Ê??gœµAGN3FGL J2141.7-3734@|XüŸ£ÀH…ÅŸ±áÀ9º;Ú¡¡¦À;ÂÊ榓¿Ó$šß>êL@ÿ<ú\R@»e€À¿á·b¾w¿í$FŐk¿Øm<7­…#¿çƒÔ¤˜·XAGNfsrq?ïý.;Ҕ?3	§²q%N>ü7¶‰«Š`>û–•s³±M?4ʤ®Îm?2_šdÓàÿ?ï|òãs­?'lº¸¡?jOcyþÇç?|å!§˜Ö?Š/nPÂDœ?"<xA?î֜Á23?Œ¤gZP?}'Úœ€Í?f}G›£s³?Ë±;CDp?ŠØ>?â¶G?ïr†‹lR?‡Ø­RI~?7†A'&Ö?;ÑeÕíý?'`­…8ƒ?‡}NÜÈG¡?ïþ×I?0[cu¿£…>ú"yMãÉè>ô'H™ÄžÑ?*¯û±é[?/DÅ6ƒÍ«?ïÖå¶?qºùvˆ!i?Så]²?Sda›QÝÊ?oõZœÅÿA?l‰-"ft?ï‡6€£1&?z^ۀ5nÉ?oÍ:¢Ý?_ÃfÒ£ ?†n,üÖ?y5_
?ïè&GÅïì?^ÿžãäÏ?(ˆõþQöü?E¸‰Zo€?fQ(µUŠÀ?^SÜ&V2ìAGN3FGL J2142.2-2546@7œà`'ˆÀGòˆÀ-'À:õÊdÀ;ÎþV²"<?âþŒ2'ð_@ªÅ[>j@ىÆã¿àÙ24Z¦¿áø'ÕE¿â@ª½áÕü¿ïþ½FSþAGNbcu?ï£<#qÊ?†cÁ¢JÛ?'g87ò½$?"uø¯pœÓ?cVã2])
?cÜܙ?ìå9ú'oî?­Á¿Yoþƒ? 
J Ö?œ"~…˜?°Ï§@f"?¤Ñ{´š?ìí2Nöw? êÄC6A£?°"9îÔ­™?š"2&e;æ? èg2ï4Ž?'NZtùMË?ëÞ1·ï+X?¦53z—%?«j`FÛo?›†Ò )k?³YB4]
?ŸÚ(Î4¿?ïߝþòӋ?gʺŠ?guÊMÓ7?c0¥ë[¶?QØmu<'¾?Mm^ÿþÓç?îæsþ'§?"PâìTïŸ?Œ;h_0?ƒãSý¦/?•#—Ç¢åt?Š:¶ïœ®Ã?îlr·–?"ŸÔ…Ηš?¡g%'±?çVe?^M(¬æ`?Üd(£T/?î©v5çBš?‰r醵Éø?—³æA£õ?~¤ýuÃñ?"S8flÔ?=YrÒ oAGN3FGL J2143.1-3928@´j¿f‡ÉÀH¡à f§ÕÀ9å)*›´ýÀ;¼÷üü??Ð9å©èqC@¾9Èxª6@•p@"Õg¿ãù/±¾¿ãSßÁy»¿ã_Ø{4\\¿Ê´ûÀ¾2AGNbll?ïÄåη™Æ?¦ŒO<ÕӚ?vµ8yÍ°$?¦"܇µ(‡?[_€;¢4?U
Çºš?ï}ˆm'Ø?Šàñqò¶–?fÉ;ÖLš?iîž*e?Šë•ËêàÅ?†òÕEåf?ï;s¾5&Ë?Zê'¹é?€G"ìÇ ?pҍÂP?Iäw#Ó
?x›'[©"O?ïÍ@?9hí¯d?Q"ýì=,?W;Üÿ¥×?›	æh?¾Š#`Öz?ë ¢
Ð?Õ¯dJò?ÃlE»?ÕQBׄÐ?A2OoÃl?@™«ç<Î1?ï×>!<ªo?mRtx<7?Röñ†9f?Q¯¿ËZz?oFeÙ½dê?gh £?ï«´i(¸†?qBU¨¸?q=C/ê#V?iÖ
sŸÀ?xèˆ1jÅÁ?d—¼?ïÕØ?­Ñ?fٓðèSõ?=º°žføî?8tîY%?s85G½?eúsµÝAGN3FGL J2143.5+1744@R~_ìÏ¢À:›?Œ
À7ykˆWÀ;™À0X?õ'–‹SH@TI,į@Ò"¡!¿ã·+À^f¿çš+FC ¿è·¾-‰¿èќüê:¶AGNfsrq?ïïÝ@•úÜ?W5½oõ-?RjÜQ­ý>?Qé6@(#?KµEÑ:í9?Eˆ¨Ó
é?ïQ].žè?"ÝB>¶?s$
PH‹?qÛuú0œÑ?'YjùtÖ?"ŒÎç3?îw};%V7?–üìn5D?–¸'JxpÀ?ñ"N?šWÇHEÂl?ŽÌlòu?îÚò@
l?›"ºÁä9Ç?sh^t½´±?wà]_ðî"?ŸÇ f]E?šˆh;õò?ïø''a)ø?G\xÊaó¾?A¦<¥Œ›©??1ڇª°?;wsI»ÅD?7ŽXJªUL?ï¾_D;̽?{kr#¼ÓE?a"–µ™–s?[-ü"1ü?xk 
;?w%õ½›ÔJ?îÜY§Ò?'Æñ0‹6?"ó¹–QJ?ŠžG!T?'Téñˆ´h?‡Âï7¬ð?ï¿]½9J¾?K¿Ê:?\ÆþO…µ?WkJ'aà?y4Dße?€L-f¨ÉAGN3FGL J2144.2+3132@T¥µà!=gÀ0Kæÿ}úÀ9©°â‹zóÀ;¡­SŠÁ?³ð˜-›µ!@A]Û}i¸@å¾@Q¿æT-';¿Z¿èL®ITè¿àvÒ&î_¿ØýNʾUAGNbcu?ïÞÓw-Up?póÿ±[¢?LÁœ¢út²?Hÿ'Ò(Ԍ?iü!PÊø?oZíd"}j?ï¶ø
? Û³õ"_?x.RÎy¸?z!ÆÂvÑ?–1<P!ÝI?FÐíðhE?îe,äŠÀ?'ÁÇM@y?3ÿÍ/g/?{Ÿ†èAëX?¡"?û‡k?ŒYƒ£í—?în÷àÝâ?•=5}€ØY?fY*Œp9?e¶C_Üw¥?§°|b¾¶?"©ì¼5¹?ï÷ª]%
ð?J#åëeÉ?5Pû¦³…²?4õ°A"-'?F®
˜n|	?Cu=t9-"?ﶂщ¨"?'t­r²®¢?c6'ǓŸ?c:˜ U‡‡?{#VZС?}Ù!ë÷X;?ïzñӗlC?q£¸<V!g?y'#rÝUy?]}¿_þ?"¯ùU·"¡?i"N¥?ï¬ñS¿Æ?sÓc,³±Û?VS
Óѳ?GØLuF¶'?'0a÷Ðb?rŒ˜Lc.AGN3FGL J2144.9-3356@&ó7z>ŠÀHÍ«ÿÍ«À8÷¨§b°À;¸£J"?ça{aŽÿü@f2R7°@\–Þ²}¿Ú‹¨-¡¿åŒv¢¾¿å•GÄø¿è}
xAGNfsrq?ïû–¶˜á?7wœ¿˜ê?,¡a¯{©?$äþÕG°?9¢»êêÛ?1Õ
À¼Ù?ï"fûrã³?‹-g5Q5?gC;¼­'?|eD?"-?…]E'•Ð?ë÷§šLî?ïXE!®b?"š@±Á›¦?‰sù£¤È<?yèƒ9Ã^§?'šú×¡?{°hÒ¢/Ý?ï®(…Á[¼?'¸Íy¸ƒ5?Fo4yi•?Kªw"ÒÉû?ƒŽ´¢*?'OE2È'ï?ïý·/£þð?'¬eêk|? (9\ô?
ÔӇ?$zÞ×(K?wL6+¨?ïÙaÀºDà?oτ,3"?R~|=›Ê?R=ú')ÊÜ?m_9²7z?ie´D³­?ï"ÃŽµï?r·D¼[?w™ÊqËÅÌ?`ègÿ3ús?~"n!ŽJ§?m®êT@JÓ?ïò¡''zï?]‡¾RD<?2[äC?u?,5ù쪊›?V&éé07X?\Án6AGN3FGL J2145.7+0717@OÄ"}À@µt@C¼îÀ9¢ÓßÅpÀ;‹N[­¥ÀÀ'(–ÍŒ@—f´=@@m`€žK¿êö¼»:[Ï¿æõ;4A¿å}©gå9¿Ì#â.‰AGNbll?ïáR}Ø ?g'¶­šè,?Er*ü©Ø?D'‹ƒ¸*ä?iP÷éÙì|?eŸ)vR	?ï¶x?ƒ	ð;‹J7?d{ÃLâ¼?eñ¬Ãª?"~"Il‡G? ±hPÌû?íðòHž?—²
Ir?–Ž>¾ùòÂ?ƒ6]¥›²-?¥©¾ºAX0?†[=,J%?Ž?€µÕ2û––>ù¡óý÷¹?ÜGW_ƒ?ˆò†''?€°¾˜éZÌ?ïðdŸšm2?UÁœLW+?9UÒ«w?4•,cay?XÏkÌ 'Z?Sv¥*sÕ?ïٚ'Ôd?lÿÜÌÐ¥?Rý'Ã|š?Qs!‡§;?lçmñ¢Õ?f'ÿK?ïI.-ÿ†w?y=ë1_ž?'àO8ÿÈ?k»²BdØâ?ŠÔ%EY²k?pp÷¼øú?ïí—Ù-¶Ð?Ta×K%>Ȳ¥ÔIoâ>Í×I¦
"?baú†",?Tx}hÙ,AGN3FGL J2146.6-1344@DT—b%ÀF|ŸïôðÀ9sñidHÀ;t•?ñþIQW¶u@þ¹+ZKÑ?ú}ÿµ,r?ï°'D"?ߦW{¯\¿ØÒùmzèæ¿ÒýGbƒò'AGNbll?îÉ&€ƒ"@?Ÿs¨RËÓ?'Jð'ù3?f'[;ù?"Må|Ó?"Û‰|`»¼?îUE[¡2â?±& i"?ˆ©*sU"?'X"ˆìã?¤_¬‡Ó?«Ÿ!•g_ÿ?ê.´‰xÔ?®ª:áßJ×?²Þ;å•b×? e˜}Ñ?»±žwh±?§éï±·?äœÝ5G,?ÀüšRÉ.?¼æö!b"?´ÊyçE˜?τ¯Òž¦?À\µ«¦•?ïcuÛ¤V?m‡¢h?ˆŒM…ã¼û?†r0*R*?},wq¤?v¶˜9fŽ?ïI^œ²?£…2òU#q?|án׍ž?•çî?¹)?7œIJ§?˜¹‡ì5,d?í=H6
å?ŸÆ8®Ô1?¥éè9Û[?"è0Žˆ?¦A"c¾…%?•¤Às‹¡?ê=ZÂÎ?¬Ã•¸Ûː?°+]ä¨.ß?šbP;³ˆ¤?½éÑæù/?ª¦íØõŸáAGN3FGL J2146.7-1527@C:\?›÷BÀFØäÀ™,À9åVI¸±À;µ5õ…R»?×¹¬%¯´[@Éª@«À#Ç¿ßíÔߟ¿è¾Zâ,c¿êaJ"wbQ¿ÌO¿iüŒÈAGNfsrq?ïõÒ?A?NQZ·ÅÍT?>.¸CÂn?<¶â÷•>'?I "̱ÝH?FÆèHúñ?ïˆÒ%k
Y?‡.'¼· ?c…ä'~Ás?f°bðæ?ˆéý'Åór?"1–gkb9?î×ñg¥šs?†Î¾ÞZeh?ŠŸ‹¾=&¢?v¾_Š Ì?—²
%Næd?']­VÑ";?ï'´ˆ?–5Ö<r&?ZÔ؏ƭ‰?bg$÷?âq¼ÀA!?•±v­Ä*?ïù²u!ƒø?E-<wÂ?.M/J%×?)èú3Üê?A¢ßq†cñ?Aim1ŽV?ïׁÃRêL?m~"M¦?RcÆ÷ӟ?P½X"‰8º?oLYj?'ù?hƒ…"?ï‡$Ã?¦?vW1žjZ-?z
FîÓê?mÿµ×?0C›át†?ngI€#¿?ïÓÃPn¤Æ?q|"Á4=?Dµþ›¼:?AØéI¿‡?s‡˜_g?p˜‹ÈÂ&AGN3FGL J2147.2+0929@PsìZþÀ@#%¿­)™À8·	)7À;?ä^¹É»?ö‡¢äß@±·Å(¾@µƒ.ž#¿áh¯¶ˆà¿è‹A".¯¿èn~K=Ë¿é}ÆTb­ÊAGNFSRQ?ïóò‰?QõM3s?PíçL«+?N…aýô#?Aù±;9'Y?;wÀhsÐ?ï–u–kM?…öý§ÿñ?e™H½ëQØ?gÆÅï´hˆ?"üHA`"+?'Fe:ÿr?î²Î–G÷Þ?'G-ùÓå?""²G^?…"Hýßd5?•ã¨‰á±?‡ùŠxÕ?ïª~¡Ï%Ë?…ß?¡©?MA.p9qß?Xl.KŸÀ?ƒŒD¦M?…†|lžJ?ï÷YA©‡g?F1'IÀ‡?G5ñÀ£Ÿ&?A£5:+?6Êð…±?0gTBÝ£j?ïÔ€7ô?q[Ø|Y?UÌ~Ëók?RâÖ«ö!?p€ß*sÏ6?lx¥š&?ï.ìê/o?…ITÏévw?ŒÈÉcßï?~哽îÓ?‡|3kã	?{ReºYW?ïîx/Uqæ?d,ÿ§?<Úq˜¤D?<Ó¯'ªj°?[ÙŠž•?b´|Oƒ	XAGN3FGL J2147.3-7536@s¼®_ú;›ÀBD-ó»NÀ7[ðEwÙUÀ;/†è¼í\?ø˜‡Ô3s@Û6"Q@rÑÊãh›¿ã†ž%€©D¿æ销w
¿èÝz!·¾¿é@«}‹ŠÒAGNFSRQ?ïî;oËGš?\à†Ká»S?TdcÕY²?X5Êô!ÓÏ?NIy¥‡£»?HFx7.Ík?°Ýé?ƒ$볘?cÐï\Få[?cz<ˆÈ?…iWä@Òp?€A×+nšr?îÞZ$¨oº?•"D"†g?"Š­]‡
?Žÿ⒠šÙ?ªV»ë¬?‰Ù~*
</?ïô « œ?aÃ8a»?ÜÁm*KÕ?(Т¼ë¸?UØBR^<?a"¾^'å?ïóʵpdÂ?S•HŸìM?Pê"¶ñ·?Pp¡ªº÷?>Øj¸L7?5sêOYgê?ïÞ6kõ?gB"³ÙqX?PŹpÇÙ?N[9eDæ¶?if•ûõBY?aГFy0?ïB}܂?=§é.%"?'Á.,9ú
?‰;(™(û?ˆ=RúV{j?'÷1P9?ïþ;à‰u¾?@»´VÃ3>ñ2"¾ï0»>þ®òÀ?*¤T`ˆ,?@‰ŒÅÆHAGN3FGL J2149.6+1915@Rœz?̞ªÀ:
Û L¦¢À9VÆu'ÊÀ;sCWm¥?c©te%_@Sz'î.Ç@Œ' ;¿å
ª
7ԋ¿çE¹*-¦¿ç›@'{Ï¿ïÿîpǤ€AGNbcu?ïåFlå G?iS©Üƺ?8sä0Ïl?> ¸æÿ?g«]~O*?h$†éYô?ïEmÂr£-?'²Ä/…¯?v¤¸Hà[?x/-Syh?'©¶¬Ç@?‹Íƺ?îKÉH/?—ýµ1€"?™'¿ìTy?‹yyÿÐy7?œôfí?"N‰]³Ð­?îµeÚû8Æ?"·y8"?uÕ|Yþà,?vuÖê?¡îòÆÄe™?'˜güˆZ?ïëÁ†¿ï'?cÊ
àRb'??rÏÎHä?I+šûÆà?`Pi0'?`L¹¬µ†Y?ï¹ò"@?z…"ßÜG·?dšÔ"èh?`äCK°3?x¹pµXì?uÄ|áE?î•ÈFÞ¿F?›~"t_¥?–è>þ×?Œ$¢4	Ö?–¹ë/'\?"jCü†?ﯩÉÆÍ?v¦QÞýû?Yцr¨?a|d9uX?€Û\Ù´	²?tY³UÒwAGN3FGL J2149.7+0323@NFâ?û˜'ÀBQ,_Ú[+À9˜ÛÈRéÀ;©¼®q—ó¿Ö s8ז@ÖJHùn@4ƒPþ¿ä{Ÿá1]Æ¿Þsñƒ)Y"¿álš¨7l(¿è|/՟sAGNbll?ïìFWÛ¼²?Yc¾Ãã°?@çp×£J?><ªoMr.?^ÿÂÅnRÿ?Ufú2P'<?ï4z{FGb?•ƒA}Ãý?uë®0Üé?€òÝ&'&?"õÅáƒ?'ÑüZ°¯ô?ï)ÔÀ"¸½?…1[^ùÊ,?…	õ'Ð?x"<¡[°Ü?@m$èäþ?}Bʋšš?î{‹Ä]?"j˜ Þ÷ç?q¸‡Áýý?jT.—v`{?¦2Äv²§?"Z4{s?ïø!ô`S?Bª.pÂCé?0F€'»¡Ó?&YËÏcŸ?G€87:Ú??f›Ù4'Î?ïÁ³cÅ!]?vÁöê‹a?_¼¤ànp?WÔ5žµÉ¹?w7$õÑՀ?sj°[÷?ï¥Z¹·O?sÛÍǤ¾ï?sÚ¼øº?etÅ\O;?z4nM6ÓÊ?mÊ[9ÖË1?ï¦ìZ~4?r|õ#)?S¶a»XɁ?D²¿ñ'ÿ?ƒÎ+ÍIÞ?qIJC)
"AGN3FGL J2150.2-1411@DMþ_ìÏ¢ÀFú?Ï"èÀ9ÉΠ£¢À;‡ìZ0Íþ¿ó9‰®¿ñr@Â}'Þ[?ýB"!=ƒ¿ãYß­5i¿âÂ:Ƌ¦M¿ÌZMN¿ð¿â‹t™É®úAGNbll?ïùd\˜SÁ?Döw¨‰'?Üqõ¯è?
îU_?H ÅõhøÚ?DH¬Î¯?|u'Ÿ?Š\*OK}?fòIãh»?z€ÿ³Zð?†QdA`,?ç{Ÿì˜'?ïUç­<¨?~6ÿ—	§`?{ì|žÃÆZ?gˆo˜?ŒÄÇÑ­Š§?wÀ¾šºê?ïZþùÅ©B?ˆœ,âZTj?½…"Ùž?Ãî©?"ˆc9«àS?ˆÿs‡ä?ïüQe+›?3z"••Wï?ÆêD?8/A@?9'µ'ä§N?1¯42Ÿ¾?ïÛK}z÷?l¬~ÔitÉ?Qƒ¡¯˜u?Q9˜°ñ?kó-kÁl¹?fQ±>Ï
7?ï²UQ/u?iDîùõ³?ol$' O?cäàÔ÷A?wEri7?Y<˜éõ?ïÙ¯.ne?bÂsoÎ†?nO_©hµ?6°ÞÎA?rÿŒS¿&'?b°ànP{ÕAGN3FGL J2151.6-2744@5PÆ3¡îÀI*èà(Ê$À:'e"'ÒÀ;Ë5™?Ç?Û/ú?\ó\@/‡­@Z€a¿˜"³ƒ´o¿êÂ#ë0¿é­"b€~¿äÔ%¥<KFAGNfsrq?ïì²iÛL?_ãþi=`}?Uö¿3
B?ZTa+î?QÕÛ¤	å?L\Q2½§ç?ï!‹Tÿ®?AEÎ<?yÈΛpÃ?ƒï³?­?•\a½¥¶Š?–5	ËPñ?î—Ä¥/?'¬ËÚÇQÝ?™Šð6ó×à?ˆ¦žÒA?¡Q¡£ó?‰Àû"ï›?ì"á?þ?©õ?A:[;?•ÙÀâ9Å?³Êd–R?¹r4?¨|çi'®<?ïø@ÒiU?E
ÌXÓìª?9|
§RŽ{?9¯>ïÎ:-?B>° Á:Ù?;÷×µî$w?ï·Ìôԗ‹?'5´È/?b'Y³èá¿?fKȒ²H?zØX¯a1"?}Ôæ9ðè'?ïKH±RQ?‡upt¦'ï?½OXCv?
Ÿ?hÓ+?‹ïނ~`]?}Kq¼X'?ï…{ÌÌn?ˆkøá"¦:?yL¶Ö°?jââéE?"pý`kå&?…<L@ÍAGN3FGL J2151.8-3025@1!Ef­ÀI`Æ báwÀ8>ŸªÀ;cá6]E?üó¥&@"¬Âc¿@	Eç#»¿çŽ:¼z«S¿íÒ_³Ä¾¿ï+¢^Ô¿ïç®ÀGXYAGNfsrq?ïã¨âÈó¶?wRÇóÖS?X©ø–®?cwBÆ(è?`!'Ss?t(ͱ%¶?ïrÆ»)¦?''lyzë.?q ñ?ïŸ?'ÝS£XCÀ?Š½Ø²Ë?‡`fø%£Ð?ëoÒ[ޚ?«t3"UÐ?¹Yi3èhH?§þL69wñ?¦P%úÄ? lH\øð?ï1O²‰™`?™ÆIn?}§f­‹?"з˜&4Å?'lIšÌÌ+?–òÏvèm&?ïä·ÄÊAO?v÷'D"D?YàŠ]SO®?`d£ã-¼?\¯ë'x#»?s1iv¿Žœ?ïÊ_N'ç?tù¿²x]?]ÖÅïÄæ¨?\Ò­tµd?sZ§"'¢ò?nóX¸Œþž?êoåÃ5@Ì?­£ŸyNíÆ?ÀÈVÆ`L?©àwv'ë?¨ò'p¶‹?ž×ê¦ì,R?ï×?¦wè3?tÔâûwW?ciK™,?aEV˜yu?eWB1á+?pœ_g[¾IAGN3FGL J2152.4+1735@RidÜY2À;±< BÀ:"曪ëÑÀ;Ï"‰G<?Óuö
°9;@LxiOò@i3ˆf¿ìn'yÂc½¿Ò¨-}‰¿×'e/뼿çÎM¸<yAGNbll?ïî\VX§?\{Mþ¹x?A¡Þ¾v¸?>vŠÌö2?Z»ï©{¦?Y4Rv…?ìžy'ç{?´ÀžŸ –N?£ÅßÂ?¢¡ïú/y?±)U÷0ã?¯x"6>†?î§àbð~ò?ˆÖd*jð`?Œ™ª¿|?v"5à`J<?¦Ìšu?ƒ™ Â±)©?ë\ìj!?«æM%u?©äø¬hm?Ÿ'º.ùP?ºzœFzÁE?¥/îÀs•Q?ïïÀæÓ?ˆJ›e¾Ï?<nsÜÈ^`?gDœ¼·Ÿu?YcHDpT?'~ƒ™7?YÈ@?š›/Š ò?…A@ª#±^?"?ƒx)Ž?'L
¤Ü‰Q?"ÑîOn÷?ïcLñJZ—?u½µ>¤J?~(T:?dFµö	oµ?ˆ :š÷
æ?q'nð'ä®?î,•&Ã8?}d›Yr?îÁÊ'?…)<u\?œ}Œ?5lk?"7êÍöAGN3FGL J2152.9-0045@Lw©Àª€ÀCÞÆ_ËA²À:I´+'À;ªÕ¥¹cÀdfÇ_Oœ@=½O?ÿ)"_è¿ê¿«4²ËU¿¯anAž}¿èòÖ¹¾0?Ñ]²eöÝuAGNbll?ïß,ZüÐÌ?h]Ï­¾É?NœaàCÇ?Jàr"Ä¥û?iOþ"ÿR?fт'-ߖ?ï v0øŠ?ñ,ÎKDO?h:-f€=®?€?4_aq+?†©W()õ?'ä_­fw?î&²qVÚ?'ï,š©S?•&—¥h?ƒþ^"~ås?£ÚIT`>)?ŠP(þ[?ïªTÛW1É?""ˆ÷Nc?±ãEŠq?+5Ò 4?…VHLô?"â`?ïïäàَ?VñŸ³ò²Ñ?=`©ÌiØ??ëÊMOI?Y¤|NÉÖ?R‹=îû4?ïܹoU€ï?i,S'±Ö?Q戁až?OÍ>²ŠîK?jSL•ÉB6?cKãoYâ?ï¡÷¿B?ƒÕ1eN¡?‰j´(?{Æ"?lÍôð r?w Ó'nH?ïñG‰V€?Y@ƒTcà>Ç#§=&†>ÏoiÁÐõo?]»ß Ú¾š?Y=´dš¨AGN3FGL J2154.0-1137@F>T2TçÀFÔÓßæ…À9:̎¹kÇÀ;ª¬ê¯5ã?î"Uk±Ô@}Ísí@é(€&ÖÙ¿â@4XLGV¿èO'²v¿çƒÉü¿ïÿíÊ"EAGNfsrq?ïÓ8n±c?t&¹¨,ÚT?MéûRù+?Q1˜iù?r¦‰(tž§?rUœf=ü¯?î™xƒc;(?žš‹ˆ¿Â?…=;¹ƒ]²?"jüEîä?¡(Ø×Á?˜`I!ú)?í¬ý=ØÔ?ŸÄüºIi?¢®½+ä"?'áÛÿOþ?¢ˆ37§D?"¶š ÷8?휇¹XŒð?£ÐØØÆ@œ?™äl<¡î?e*ûKþ?©Ez6ì•? ÌñVa9?ïÜÁZ'?rJÃ]cc¢?RBÍxüèŠ?ahpÌWÇ?j>ûûzë?jÆZtÅ»?ïaSFpt)?‹lªHô?zŸzþ¯?wHߓ^!5?Š[qJ-S?'°¸K݌?îJ^Û$ç?šÃˆš1³Æ?›¤4q.'ü?ôîϸæ?›ð(•¢?"—G$™Í?ïZ¨·!?ƒ'çV$?…÷¬ÿÞ(?qy17Ì?ƒ"MÊ룋?X¢¦ÜçAGN3FGL J2156.0+1818@Rº6ŸÏ=ÀÀ;Ê	 '²À9ôW(ÛÁÀ;š}=B€®?Ç`d×ù"C@¸]?÷î?þ `"=µ?ïüà*D«¿ãÿl(¿‰¿ÓäŒ&iv;¿ãÓ7m©"AGNbcu?ïòíüa)?VÁ{¼6_?'‡0s}Æ?#M¨ð_?XÝ>:Gx?Uu!ÑGA?ïÏ+‡ÿO?Ÿä)f©øÏ?}êŠKÐ?€>3SSãý?–a_åoD?œµvU-F?îòÍëñ+?Š.Vï>Ö?"°
üÀ ?sϨ3
O?—N=!^ú€?†öÃ׊ßÐ?í>þÃiø?¨í.Ÿ®9A?x¶Kß-Ú?u¨²W%äÀ?¶J£Mˆ°$?¨FéÖ?^²?ïúä0ÛXð?:Â×9ñÈÌ?S/Ú%?vùæŒ?@ä×KÂkÑ?7vۚŽc?ï°$^Ú?"ñº?õð?f²â<ãò–?f>±_>Å?|šü¶@Ž¦?†µŒ@?ïaÓ Œ¹?…m`fÙ9(?x ëꕧ?l.6¦©@?‹<‡tòÓï?ƒÏMäÞ?ïGî,ݝn?…€€?–É?lõ'¾	4º?VîE[aú?"cˆ++S ?"]Ù=‹3JAGN3FGL J2156.9-0855@H.­@?‹0ÀF HtäÀ:t䝣êUÀ;Æ£iüóÜ?ÁÜ#¾r@M¯gQî?þm'Ԇª?ïñ½øÒì?ë£`Æ>F¿è'ßSª¿°¶¤cC"AGNbll?ïß+"Xü?n˜€ðKq3?H%a«ø?HŠrGŸP?j˱'1a÷?lE$ÏXõ?ï9/b)|?¡¢b'«Ê°?qlÁð]õ ?|pÁû4ٙ?"©>B?ŸµPß_"G?î=²KêÚ?•®TÝfž?˜²ÐH?Š÷yœï§}?Ÿ–æN¯9?Šw
C-¨å?íd"cýV?´SèþdR?¤­¾VÌÇ?±4Z
†˜j?£þ	ûi]á?¥wìOòF?ïòL¥8øß?ZÓÇ9½?4—(­æù|?6<ª½êè'?V@ëŠ)‰?WÆfÎ儕?ïÈVêâ%h?{›ùV~Íø?Xe€êÎxõ?V Ùó?u»*R)é—?x1¼w²B?ï1Ýâb¥?†-ò}ôf?}•Å93?8–£àºS?Šµò¾ï'?v!BŒÃЀ?ï¢Hò¸á?"ö'Ç\-O?eއR£Ê£?atB¸÷¸?ö!€…+?ƒz€û«AGN3FGL J2157.5+3126@U0m_êKcÀ2=²?'ÌÎÀ7ž1œZ>:À:ôŸÅ,Å[?ýºOq­A@¬:ŸŽ%G@¢ø{§@¿Ý9: Íâ¿ã–δ¿ û¿æ_8`ÞUû¿ê¡¯`¼iŽAGNfsrq?ïJ	d
t+?ðõ_¸ÙB?€ì(ˆ?ˆò|#?ŒßºÓ4¡Ç?š¦FÝ&d­?ïtÕ ¹|?¶<ÓË¼?q||cצ?wøh)?ŠALcvk?†Žb€i! ?ç^iº%M?³£")?ǖ«6¾ÇÀ?®âoppî?¸_¶DCRš?¥YÛ0ÆO
?ï§~n<k
?Š Ân)GZ?O1<?f†¼WÁ«Y?"/±[ʱ‹?‰¿6uØ«E?ïUI~VÐ¥?¬FÜþD‡?wíÕ8Ãÿ?"K¨áÜç?Ž¶µÃ¢ªÛ?«¨cn¶ØI?ïÊÅðBP?wæm@úãã?]ÏéÁ ?]§GS"ü?s‰X–]'¹?r¢X@gˆ?éŸXc!,?° û£'úp?ÀÔv?Þx'?««bË¥{?±\Peð‹?¡†j¼Ý!¡?ïì­9«ê¡?fèy8??fî2G?BKnÓDMž?^Þ2¸ªz?eHŒžLô]AGN3FGL J2158.0-1501@DOs€*\ËÀH ö½À9+äŠYÀ;"C/Ш¿óòúX¡,@^‰x9M@'Õ`EK¿ãyGë=|¿ãàã»âÕß¿åu(ÐGšb¿Ûª{4åÍAGNfsrq?ï÷.ô	¹?IúâwQ'o?*Y×òŸ?'¡hf¨e\?LÃÝ°ömB?Hóžý?‰?ïš0ðZ=?ˆM6½Ìì½?b°"íCv?rÔj²ÿ?"ÇžønµA?Ôx™ð¾?îàìÒ%Ò"?‹ C@—Uå?‹ÿB9ï¶?|Uüi{!?•âļÐ-ê?ƒº#*f+?ï¹°&±^?{ËM'ôc[?
CÞÿó\?#xCk"h?vµÞݒ5?{³"÷«²?ïü¿¢Ü}3?5¢Ù>§¡Y?,;Յ'è?²˜aÈà?3w؜ܯ?1Êú­Â
¦?ïÜ$ñ†?m>'ôL5=?Pñ‡H‰ˆ·?P¸W\v»+?kky»ý ?gXéF¥?ïŽç¨Sé?qà¿fJ"?yo|t?gÍoš!ÀÎ?õC5wB?d&Å»ÝM?ïô)†ûÌ?M'Æš'æ>ã!Í¢Æ>èàq¹ÈÙ?W†¯ÕÖ·?M€Ù@7ýlAGN3FGL J2158.8-3013@1º¾`"‡ÀJã?ÕØåÀ60Õñ8¼àÀ9Ïù‰Ä:?ðÚº1¦k@µŽM5<ù?ûCÁñQ'm¿Ò
¡ÞPr¿Ý[4Z5窿ٯ ›¾7¿Ú@µwp¤ÙAGNbll?ê°_C‡i?ŶpûüÌU?Y?«A,à$?]fóÌ
p?Å
C+ñû?Å¥"Om?ï¬/ÑÝ`v?ƒÔË Î0?_fÑtÂÊ?e⾫hÐV?1efUÜ?€wϽÀ†î?å—cásDh?´÷)?Œ?¡¹´²Î?˜ÝJ[^n¢?Ò¯¡§<x?´0¼e•hÚ?í°L"E¨?­qûˆá‹W?"¿›C
iW?8idÒÐb}?²t<'†?­k÷/Wù•?êöKð‹ª?Ç?B݆j?gšû—zã?rÕÍOr9É?ÃÈhš@*?ÇÁ´ôF—?ïáUj/±?k®ƒ±ŸN?Mûë]/·?PoŸZÝ
?g+›áåá?ewÓIáD?åfˆŽÑ·?µ'šã?¤ŠZËùIJ?œƒÃJ*"?Ò¢•Ñ&è?³å£Z¢?îõ µÂš?"­Õ@Ût?*?iðH"5?)tàš'"Ÿ? "6‡•Nö?"«1"‹AGN3FGL J2159.2-2841@4<ú?̞ªÀJ¼ .ßÀ:¨y0nÀ;´ÆžµbM¿áäò
¦f@Øe-VOm?ÿSßûþ"¿ê³A¥*¶&¿Ü1''©Ô¿Ò	nÕ1˜¿åG‰óD—AGNbcu?ïû}¹-!?6ºþtÙú? h,4"t?0
˜¶	?;Þ"õ§N?2 "ŠœjÝ?ïyòý¸ýã?R9â
¡Š?l÷?ê_/•?}·ÉÃHº?ŠEp§¦ÛH?‡æÖ¹4¿?ï<ûkp¼V?'	ü¢
S?<Ñ$QÃ?m­¼£R?"T
tÛ?zÂv~C?ïVäé#E?‹ˆ§ó"Nì?I; D¶&u?R vËY?œëFZck
?ŠìñL·Rb?ïý±%M?%r˜twP?…ԐÇ?±ÆDËÖ$?,i
ÕÖr?"#/–€?ï֋"*Ê?oG†í¾‹¡?T€‡È3|"?RŊiÍ†?o4(Ù¿6?iXDpbŠ¯?ï¡ÌÚþW£?i>2®¾šá?s¤–`@Þ?`øáHÉä5?{tü!Uj?]O	ª-""?ïË6A?b‡öŸ%??9\g(3@9?-å9«ºÍB?xڞ8'Q?a²ÁgÖãAGN3FGL J2159.8+1025@QFàà¨.À@ú0ߛÜjÀ:þñ´
À;µu	—Xw¿ÓK!ÄÿW@ùô+¶g0@% Jù#¿êS?V›ÜÚ¿éλžônʿȑDá[z$¿ïï{¹ðã>AGNbll?ïóOgû?Sþԉí³?B,ÀØÔ&?CØ qóƒ*?PKža2n?OPD¥HŸ?î¢Þ!
k?¡¿ç_já°?‡Ç…T"Ú?ŠáU}²sµ?ŸÀy4ýÁ??™ë,`?ì²~{õ³?¡±Gês?¨düýî¸?•-õ~M²?¬sC'õí?—·HÑáü¸?íêU1=mQ?¥†û 3Œ€?y¾¢[?Ý?€2':)?®(µvñ?¤NzüêY¢?ïóù À3?Rœøá¸<?Ag"sQHë?@à¥&Œ?N³û
ûû,?M)ù±‹×?ïvþ«…ï?=Îp$¦	?wы³ßäT?{ÚÀ"'Å?†W?ì5?Í51Íóâ?îùJÀSÔ?•¨~´œòm?¡87lt?Žù¼Gƒ6?›PgÖ»Ô{?Œ•÷Žòk?ïÏÿZã?~txwàâ.?iúnÕývY?b7PÒûm?‰dŽS¤?z·¨"srhAGN3FGL J2200.2+2139@S'tÀ0ÝÀ:6_7üÀ:°àÝûÉÀ;Ý`ÖÚlÉÀ.Ð ¿=B@ŽdŸfã?ÿ£k_I'™¿íx[â»ã¿Ç	$6@-í¿Ø]Ÿe`'¿ÒQh3VTÝAGNbll?ïôÓûÙïd?OŒ#¥¸N¶?+…›Ë2·€?% 4ü¼.L?RçU*$#õ?MŸîTÎ.?Àë¡?‹e\iý
¡?kkÁ\·×?|Û!¢/Ëæ?…¼xo<Ê?'`Ü«"tm?îÃwùX={?…Á¥Ìúþ?‰U0hf?r»è"Ï"z?›ý±?T^?€û¶'È?ïÆL¾Û®£?t𺋁Pì>ü¥¼È8ãÌ?ùÛ«Ex?|¼úê½Þ¨?t魖nF{?ïø´??äz??Âtî	?"B,•HGá?ÞŠA?HžxPÁØ+?=PÇ5D?ïØëy¾»p?l
ñªEŒ?UBÐ(†ºÏ?R·c;‰"?lsE¾bÀ?e¢4Ѳ?ïiÄe†RÑ?qrÞ@Õð?|Úw"÷?b-`6Ô®ë?‡!ªÈáÏ?gƒHàž¯¼?ïôgãéôÑ?K*0|Žà>Õ3/þ§ƒ>Ó-{F~Ê?Wñ|?K8ï{ž•AGN3FGL J2200.9-2412@;}"V!uÀIÓÝà‡kÀ:H%"ü|À;â½ F?¥½9…'‰Á@e›»2@¡³_¾V'¿éƒëûnÔR¿ëuÄÓ·«0¿¦õ§•
vi¿ã)åz©Ð…AGNbcu?ïú;ÿÏGj?EØï˛?	ù+]Ý»?
PÀ±`?DÎÁ¥ÈÀ?E«?º?ïsˆùÁÖ?Žà‰wurí?l€'ôNE?vDÍàú?‹ýœÉ/üu?‡é¸äå'?î£eYdäö?á;ø1]#?‡΢FÇ?sc"Qtù? ¶Á /ñ?‰/|m¯s?ï-í_O¬ø?',œ rl?IÕZ¾—9?RmnÛ{?™s©<qAÙ?ÞãÔ9?ïüþ3Þ:?1;á'	–?óïùâ"?[¦©Z?4ïâù4÷?/ì¼h)d5?ïÒ·ŒÁx?sl3"úÓ\?UYyëÆQ?Uˇü ?qMÛA^?nŽÐä?ïwx›áâ"?sÓÇaøö?vN³÷Ó³‰?dx±Ÿî?†ú<…Ë?p‹ŽÙÂ?ïׂLÃIŽ?hŸÏ뜏þ?Cd6ÛálT?:·°¨9Ã?qÒRÂÍt?gKSg'€AGN3FGL J2201.7+5047@Xi"d¯À^ƒ¿èÉÀ8).‰À;5/»¯n?îkÀÀSJ@r'2Ÿºp@¶Óàg^^¿ä$`gÒTÕ¿ç6ÃÝ©­¨¿è®n4]w!¿ï3Š!oAGNfsrq?ï½4zä€?uÃٍ=Sg?q® ãJÆ?oßs›•·?o‰¶H60?fãÂHk©ô?î
V"¦¤?Âl©Ìlª£?å.¾'v?•ÀÞ~'[?«]ðÛ{º?ÀÙ"}zÌq?ì-Cðù/Š?£¥ÔöóÊ?®iŽ‰Ò•?˜t±?®Â2dã Ð?œF¿¦:?ïû·Æo)?Rݱ"Åi>ôÇúÈ÷§g?yJ šO1?BúáÚÔò?Ržãµèsã?ïËùæ`q°?tgGñàõO?qÃ<'g?ošü€N°ñ?aޓ^Åé?^&¥9?¦±?ïŒX"Ù?ªï$·Ãœ?b>¾N&K?rlŸGåá?ˆhºW%?©ìpgWcO?í»±ú
^?šébgzÎØ?¢båC	kÄ?ÐFÍñoV?¡â	ésY?"©Z¼?ïÿHöûÕ?/qš˜jè>×äñQ®a>÷®ëHP³C?bÓl«6°?/6<ýU†¶AGN3FGL J2202.4-8339@s?÷LÀ?¼±v/À8}¨'j¨ëÀ;³¦‹¤?ú>ÿ'ö×@ºæ´Õ_C@"?(ßÈ'¿áðÆËÅ«¿åÁªRàˆÓ¿è¤ÃðÉðé¿ïW¶ð9üAGNfsrq?ïMÝ#;ï?"|ÕBÜ?'ÑlÈûA?'ûqåph»?qØ~EÓg?j>rüÖ»?ïQ÷1i?'cÊ<œ ?r»œâØî?sNí£Üé{?'.ëNó!?ŽÊþL"ÚÒ?ì%­AIÔé?§¸f§t'?´Ì¶&˜>?¢¹"Tvvj?¤¿¡¢ò?˜)õ™Ó.?î²ÑøA?Ÿè€«Â3?€´° Ñ?ˆ9¢k­Ö›? ¥´Z@?œºíÀæ?ïŽ%ŠËm?†¬¿~?'?ˆY7{W¿?"¤TÞ~¦?aÆuÄ¢Ñ?[˜­´üE?ï³ÕO'[?~íãxÒ¼?ew˜"ŽU?cÝ
 tË¡?{¹ÈüD?xHQK£Ì¶?ín‹pXz?¡Ìî±~0À?¯âuµ?'É6"^?ŸNPäÍ^?'·Og:Y•?ï"x'Y
]?'ݪ›l©?v܌45¥?nØÎ
)¬?½Íuçª?€Y°‰÷CAGN3FGL J2202.7+4217@W&@_×,À$á'ÿùJÀ6t _ñØÀ:…nÉw-?õôò°·@0áhv@ã±jƝ¿á€…15_¼¿ä©§…âÏæ¿ãÚÓíõ³Ã¿å±ë`œßAGNBLL?ï-†´Ëµ\?œßGñ¶Z?EÛsP8?Gš6®û£?™ P®HqA?œ­ås:H÷?ï~Dz>›­?)-€(ÊÉ?oô?ŸüU?zŠó'{íM?ˆq¾
‹;¯?ˆ!¶–Ñÿl?ëI›¹ü²æ?­ÜÕɽt?RWŽýÌY?"yÚ·qõ?¾^ŒNø?©Ë[©^?ïêÌ`°ß?o¨X+•d>õ§6ÉÒ5Ý?
#˜
"9(?eP§|w?o¡ûÎÿU?ïÇbïRL˜?`Ç®¾c?>eö¸?>!…Ûn?zh)	8¸Ù?¢úze?ïÐYõY?{Šå—¹
ž?VüA'óq?Xh 'âã?rô¯
]?w¹eöÙ­‡?í"
99v?¢™¯@Ž?'¿vojhv?Œ±Ò¥c?­ßt'#c?Ÿ‡ÕÌШ¤?ïü
"ÔÒf?HmGª$€²>ñ"	
4¢?û1ôˆ›?>•ºiý?H)šßèþõAGN3FGL J2203.4+1725@Rëà
ò1À=£GàiaÃÀ7»Šˆ"ž`À;Šrµ)B?ñååóö@ڜ#·•-@QâZþ~K¿ßð0$ò¿ãðk"LD@¿æ!ÓÉã…ÿãSù¼;|zAGNfsrq?ïñ»ìÕ«Ä?W 4gš'?*bµOÈ?("¡ô
?Y;âØʀp?V¿$ùµ‹?ï1»†JÕ?Š*‹êtZ?iR¸v%±?{Ã(–œ™?…Þâø(k?€öÖ¢—Ѻ?îo:¡wś?˜š@¿€"?'|•uõ/?‡í¥Œ r,? È«À?"\Øçðç?襤âÍë?†yñ;I¶?<¦R4ä6î?Lz1é…NQ?…ñ"Èȇù?…ÚòÜ)VÔ?ïú!z՜?A§t_'4?#ÕcDoud? A'¬<Q?B"ÀŒìæ??–AIƒ?ï×1¬9H:?nó¯Zîº?TÝ¡Â?N?Qò§Õ'
)?n_'¦sÖÁ?h"ÊVp"?ïA©þ1Á?ˆ%Âtäk?"eQÛ@`I?}G'ï=Ä?‹0J$Û9t?'è¨Ð.y?ïíãOñ?aØ:Ó^a?,Ý|Ÿœ?(iÉ­‹É¯?`NØd_lù?awÌúøäÃAGN3FGL J2203.7+3143@U¸¿ÏŽHÀ2ރàÊ°"À9 Qðœ5À;Pf͔ÀŸPõ-¿@'=Ì¿5à@†‡_ZX'¿çšøO:c¿éWÝ÷cñŽ¿ïÿÛ¾"_T?ÚW·€¤AGNfsrq?ïù$a¼¼?GÎF?7DŽº|1H?8¼'ÚÏ×é??oPö^?@ÜÍӂ ³?£/Î?"YI¯à!?j8òr Fâ?l±£Zöa??ƒš™t1â?€v˜Ë+ú'?îl/‡=\¾?"£À3î6W?ŽÏMIx³µ?ÌwÜí@µ?¡‰48ð 4?'ÇÒÉkT?ïԑ¦˜?|JÛàÙњ>ÓÉd¹ä}>í|³´ï?u²_)ÝÔ?|I7‰±?ïûœÀF?C¯Hy":Š?,wq¤C'?1m²]=Â?8ïf=6…?;…[‡4£é?ïÕoAMË?v("k·Iˆ?UîFS¨Fü?Uá1®¿'?oým!ñ?rqCÔáY?ïDL¥õób?‡ƒ3)6Õá?'ïa´¿R?Þö/È ½?ŒÌç4W?€^2rfw?ïú#±½Ê?G8ÉüUL@>…®K@¢3>"F¼h¼?Gpž:ð¼m?G8R'¨'AGN3FGL J2204.4+0439@P.lŸÐë?ÀCSçÖyõÀ9îévQÀ;Ãr°÷"0¿Âîªzüö@^Óª¬±@þ=ß^ŸÉ?Ùlé™BS¿ÚB»ú "R¿ëM豍^Ö?²uµ"(üAGNbll?ïÖȃ^f4?ríwÓ{[¤?ejÏÌòdž?lD–Ä
q¿?c̬ð$G?a®½sº¡?ï#fÀ?ŒD* W?fLJ[mäà?gO¾ò€"î?Š$µ³cl?ˆÃ9gÒ?îÿLj«‰?›Eג²üj? úU÷!lß?"7Ùæ.Ö?j"gµ?‹E†Üxru?ï-@ùM?–k]¨´?Qç9£ýX*?^ßÄJA£?™9m>YÈl?–
MýV0?ïò­aÝ?WìÐg|â?E
yÅ°ý?L×õ­L؞?Pßt¡?Ld†7|ùÅ?ïØD‡™fï?jãÂÿ6àö?S=:Û?L?P¨u¶ç?nïUŠ	}?e,ÉĨ
Â?ï
WNñTÁ?èîn¾h?'ågJ²?†‰Ú½Xï
?‰ ep/?|ÑP˺ ?ïá°¹h8p?k©F_à»A?$à['ð©Ö?%TGÃ~p?m@µdÎ?kQMÅÆ¡LAGN3FGL J2206.9-0031@Mú¼ßï¿@ÀE6ö`D
vÀ9¢T™µHLÀ;ªf̽³T?ÐXá"-nÎ@Ûhêz1Ê@üâo\¿×âK€K¿âæ‹Ôx×q¿ãï/Z¶"â¿è~ %ò$mAGNbll?ïæØP°éå?_ÿ»»C>Ä?VC,lg?U1¾[¸?\@Zź‡?T+¾=ˏ ?îõRDõ?œüc[ý?{·´^ÓÉ?{œR©–¢?šgÊ|€þ?™ É·å!<?î¸qÙa/Æ?ŽMØËÃ?'¶šQ¤õ?"÷ÝtÕ?–;*‡ïÌL?'! úçk?í"8¨×¿?Ÿ¾_^¥ËÙ?‡6oǛÝ?ºØ¤3Šù?´kvt?žÝÃÊW˜?ïöÝ*´M?Fkkʗ7®?>ÈdßQ!¼?:‡#j"p?E'ŒÐý?:ò55ˆ?ï®,E$Ĩ?€wÌ~PA?dâb©w?]PIûÀåí?~x¬,ðð?|¬øü•6?ï}@™¼îÍ?~BÕ|ó•i?é¢K¾ø?y¼þŽëߚ?3ßòî›f?l'¶IRWY?ï=æ"h"?0j1žFö?vèÏR)Ã?`;ºm[Œ?'‰5Ӊoú?¹¶2j*'AGN3FGL J2207.8-5345@u>…ߨq¤ÀHøm¾iÀ9ôÛö5À;̪â—9m¿÷?´öÂ?@\Ý%µ@ªå_ë¢ü¿ç~"ƒ
¿åCîÛ{¢t¿éjÄzÔç`úû©ëAGNfsrq?ïûR"ªúô?:ŽÆ‹œ!?%=IW¦öË?#çõ÷É­#?:̶½Ø?5ü'V¾?+?ƒ™­·­?bÌÞp[XQ?g?'Øî
Ž?ƒc}¨Í>7?Æ&ßû?ïòúwÄ¡?ƒv©.ÖåÒ?…
÷Ù©l?pyz».4?"œ%';_%?€O4Êý´µ?ïåŽQçÔ:?l1±zwD¤?fÊJMW?$wM}i¥V?iÞwžŒèo?làšŽ$?ïýŸîÐá?*®!w˜Õ@?~1½t
°?.½'"Âþ?(æèo—J?#õ·œ€?ïÞÐ
°(
?l¿€›âBW?PÕé@tß?Q'œf|…'?hÄýºœCÑ?eÓgqWsî?ï 4["ê?tzÿ—{ºg?v§±·«þû?atWP­ò3?€äx?q7\DW?ïüTÉR?E1umÙ¨f>à°]' ?-£áþl?<Ú<%8v?EÚFý÷}AGN3FGL J2212.0+2355@TŽH¿÷Ò4À:©?ÿÊPÀ9}K…9À;†ûß	?ÕKêßâ@,þ¯çÝ@²Ô (>Ž¿àÓý鮿☐MH:à¿ã«Àsß1¿ãr`†Â@FAGNfsrq?ï¶Òc~n_?€ò³c1º ?a£EÀ*´S?aJ»X¼Ë?{Å+oѾ^?|çÞqHe?îPxs.Jì?¯eµM•=?ŽMÍ,1ûê?""ëÜrâ??£e€WG?«T1³ëÐ)?튇¶uÐð?Ÿ,"Sf?Ÿf=X/¶?îA…"%¨?§¤f®§ ?•Ö¾dÀy ?ì<Æ.øç?¤'¶¦vÿ?"óý«Ky¤?ˆ$v1ð?º1a!¥d?¢ÔÁŪ,?ï뵝Üy?`\	oE ?HÔ»'5Äû?G@Ç£^î?\*fU&|†?X×iuDéª?ïv\n§
Ý?–,
¶2=?tBÞI~?w'<´?ˆGuSvò?'¦'ÑSo>?ï2*‹*&U?†@´	¹:"?‡}Ê[-x3?|5ýTuá?‹÷'ÌŠ'†?}$Ӄµ?îÿM]ßaØ?ƒ–MR!ï—?€¤²|'?fÜí|%ݎ?—Ãû'2ó?«ÂuHAGN3FGL J2212.3-7039@sôî²ÑÀD‡"€,á
À:${À;´»¶úÓp?ìû–dìúÑ@9`؇ëò@}\¬~¿ç£ÿ¦5UÅ¿è^VÚN·ë¿ìJ¦b2'½¿ÙaÿrAGNbcu?ï"-3X·?"öü¼¢´Ö?x~p\´?zU³¤©`k?}yùló0T?yæa=Ȑ?í¼Õùœ8°?¼þ»-#_è?—^kÔ?°Œî06ä?¨ƒ'hŸ[
?²;8eº(Œ?ë^µi%?¥û֜ µí?­üÚ\lÆ?˜âñr
Ä?¶"áÜ¥ô?žéíŒ8q±?æÖGwÖ?¾"¬ki–®?ºŒbø¯?ºŸ–;sÒ?Ç`ØpL¡Í?µ"x¸ò|?ï¾ìrY?xQkÜ2͈?gµÈ^‰e?eGßU!,é?u%?Ý}?r¶ø«:?ïWµvÍoh?¥†ÀÀMX;?~ÎË4XH?—Õ&ÎÐüë?Š«<£,<	?–ÛoƒÄ»É?î™ÞŸp?"ÛÙE†:û?›ŒõœNÕ¦?‰tSàÏ? ïçF/@3?‰êšâÇ?íR~ÊWÊ?§O‰ÔJ\ª?¨ÂÿÝZ–?¢*V!Â?¥ÇØ8"/È?—Ã0|AGN3FGL J2212.6+2801@UK2-LiÀ6û.Àë­À9ðÑ@±¡À;Qøñ?ÞwՋڋŸ@
z£?	Ö?ü¥ôÞä§_?îñÇ53=š¿Û⦖ŠÏ¿Ïáì"b½¿Òې
m•žAGNbcu?ï<oê@?‹cŸhŽÕ?e⧞wÌ?cv—ÍðÅò?ŠnëT©"ï?‰hvº[+?îÛaüä?¨l®Ú'Ÿ?€ò«¿&»?"‡Ûe¼à?œ%ÝÙõ?¦åZÄ9?îAÈæýê@?'eŸµö?'ÿ(ùû,|?€'?Üoà?¢cÝ"a¿?Š²_…02?ëڈ¢%"I?ª×Àœ—ï®?ƒÜºp?†Uä8#\ü?¾°#¯î«Ö?ªfkÐ_??ïÛMîöBg?o­[z"?HïêËý'?MÁoƒý~ï?nv"Z‡U?jãH%€?ï›3}Ž~¼?à^¡Œ\?iFUi/š?mžÎý¦§?'á‹.Ÿ‹-?‹7¤ý'÷Æ?ïPîႀ?xž0pJì¾?Êxs¬Ÿ?jÃzÆ=?‰ú"	¹>?qðÿ¯ì¢ñ?îÓ*m?MBMäV°?{Å£Ð:?oÉuÐþ?ž©V;{>?‹>Òx³EAGN3FGL J2213.1-2532@:UC_Ñ ïÀKQìàh‹À9™TpšÀ;Ñ&çËUÔ?¼ŸáA+¢@íÓW«c@`e@ ¬s¿ãŠn'!¿åÌ3[t¿æ¬K¹xz¿ïÿõ•æ(5AGNfsrq?ï×0üª¾Ž?~V*ow"?TšC¹™cq?iº™;IZÿ?náe6ðÀ?x̵èÑ?îl뀗.?¡àÔÉK?‹ÏEÇL!?‰P½"Xò?¢=v‰m?›É,,¤eà?í—	·òº?Ÿ—$ŸF¬¸?¡Ø4ˆ="Ä?"Ìe(€Í?¤·:z‹r¡?˜/ÀÃò6'?ìÑ<Èc?¦±é4¡H? N…º™?–þ†Æ<Á¦?±oø¸pû?¡®Ïûo;f?ïÝDÿŽk?›í0Äü›?CR-â'H˜?R=Cı8‡?mætÐÙe?›—¦I¤f?ïm]!¡?†ø"ªðÇ?zG×¥Xî?tªiŽL©
?‡ž–Q½AQ?€;FšžT?îàŽm
? yQ<3?›é)Jj÷?'ç͝ñÜÀ?¡hƒ®%?š5RÆ»?ïLåN¬i?ˆ4)D WŸ?©¨ý©}?|ζI'?Œò û?[?Ù™öI™AGN3FGL J2213.6-4755@uÀAà?pXÀJ"õƒ¥À:Ú'ˆ-aÀ;òABÀnð?dz¼G:ôj@ÇÉÅÜB·?þ;þÝÁ¿èeêG(ó¿c>"0hê¿äxiRÿ×;¿Å1݌|iAGNbcu?ïÚG¹twÃ?h¶™5ñÖ~?EÑk±´Ä?Cu	r[â?p!õ龯…?fÑ	òG¨?ï+lƸò¶?® ß%ma}?r:À!A
ÿ?ƒ£ïzη?–·iû¸?¬J½Ï•W?îw¾›?‹}›uê?Š®|ý?zåa>? I8~ݼÅ?…tÜ×ÏØ?î©6-Ÿ±?˜'a?{âöÏfšh?€÷9
6ý?¡ð>M	÷d?•lt&ÖI?ï튈ì?g¸^®¯?8ü;Š"¹?8«ð7óõó?_Ä)eÙ'?f2«ç?ïÇlLHG?'á/iÖܑ?]†j÷'P?u•ƒ 7®D?u/	‡X?‹U‹ÔˆM¯?ïNr'KÆ?|°Ñ£/^?'L²vçh\?p'\'bx?Šû×7?t:N£X·‹?ï¼'³£0?qIŸ«¶bŒ?]'z,ì)?W¡_ñ¸*³?z‡Ç'n?mE¨e˜?çAGN3FGL J2214.6+3000@U¶¦ßÓ9ÎÀ5ª¢_:øúÀ8"kp'b"À;k/¬•õ @1Tc¯}@¦ÃMÈ
?ûÑE'ñ6¿œ³š~V·¿Û˜Û¥úó¿äºˆ‰&¿îwe_*\öPSRPSR?e·ý
Ãڋ?cóY ©(
?ïÜÿ9Z?l¤\;¿ê?Z'±Hgn?YçñØß?u'Ë%ªE?¨ˆÌ(ùM¨?íI3Îõ­'?¹|'ñs€?´^4×Ë¢?¶9Ìká¢?–iÎQ'€?ˆº±ÊÆjç?íS]î{Pâ?žCɒân•?¯•9íÊcà?™j÷
R4?ˆMïb~m?~*'R6v?î–ò=}A¨?˜{ŸXh¤? }`R e?–
"€9¨?_ØnDýŸ?gS³|]å_?ïáœàÿg\?€©­±Q7Õ?\íÏÓÉ|?~1¬%ÉÑ?wy˜9 ŸB?‡Z25
QB?í0ÿ£Rš?¶ŸJݙ¯±?µV~8€?µ'µ…(J?£óœMË?"ý½×ý²'?í)Àórz? ²Ã4"Gª?ªWý0ž—?˜$]ì~Ë?š<~shü?".RÊ7|/?¡É`S?†H÷9ƒ?"}oJZ?…_¿X"´PSR3FGL J2215.6+5134@X÷ÏÀ1³×À¹vÁçAÀ9žý†¨üÀ;WÊÆb?þ¥y+û¶@)"×ëŽÚ?üÕJœ?Ưåi'I¿Ûön+¸ý¿ä\z&.4h¿îÜ)µþLPSRPSR?mj®èêH?d7O»ì¸?
í*?ƒËA.÷?üÒÃ@ºæ?€ç»Ò/ãu?q^¹QÐl;?€0|4±ö?ç	²*€@?Ãd˜›lØp?ѧ ÅQ1?ï°î?£K–èu†?'o@¥mª?ìS¬_ç?¡Îåmçëà?³Ú@­?›ð6·¶µë?»ZïØÉ
?¢c£´Ï?éÕGCľ?­&!q§¨Ÿ?µúÖ4´?¥}\òÖ>?aƒã²"üÒ?g`¶"å%ë?ïÌ	}yŸÌ?zâ,Ü<¾?q9O_—Gã?t;€­¼¶?‰?ïXz?œµ-ýFð³?èZ oäû?¿-¨3);ý?Í€º
äq?»ãŒ
â8;?°‹J'Ô?2Û¿ð?ëȍñ'S?¥CbÞÐ
?±0	îLk—?›wïÉÓ¨q?ÌëÁWÚ»?¦ãùX(݅?ç7ð‾+?©Þºòú?¨Ñí¨L€Z?š¯.YÄ<fPSR3FGL J2217.0+2421@Tâ5`4>À:u§€)ÚÀ9;ٕ2+ÌÀ;‹õ'¾´?ä'ú¾z@'/ó7Ŕ@¸Š`¿Z¿áœ坠‡¿äÔ]eòßA¿ãªª=€¿¿àãšæîAGNbll?î/ôÈÐz?°_QŽù?…¨mÐp£à?‹fM6ˋ]?§–—ý$gð?®cðÆJSk?é£Ö±¨??ËÜbÝÖñz?¹3ƒüüE?€å©Î¬1?¹­ÇVžÐÄ?¾']¾µ ?ëc³áò3?¨*vtq.%?©(ñ¿4-»?–_ý{T??¸MèÂ>Š?¡y·Eð*?âUÒËGM?¼oš 2m™?Á¨6÷ý?¶X–,a9?Ò̆NkÑh?¸ÿ?j	é?ïÁ£µ£?°tfK#ïè?yD]"ŸÒ?"ñ¯LŒµ*?˜–´?•Ê¶?°˜}_³6?íÆ,‡rzœ?»ÆYã´? ñ…~Y¢3?°ã$#I%ü?¢«²êÿ?®"B½BTß?îzº…;W‰?'"eq+¹?"¨ñë2~?…µ'N"¨?œÿ½m'Üj?ˆSØkÒ¼?êŸæHãr?¤iσëš?±ék•¯'?›+z…–Ó"?¹b#¡õÓ?ŸÊ@FZ›AGN3FGL J2219.2+1806@SÜÝ?á—_À? íàBËWÀ9ö-Å5(×À;Ålґ2¿åŸLv{1z@Pš¢-@	qŸŒ¨¿áöͅô ¿è^ß®ü­:¿æˆ#Ó¢\"¿å¶"ÞAGNfsrq?ïïe졇?cõšøô…ê?->ñ¼ ?1T qwì?]ŒHòíU?bq"ɂç8?ïr3‹P?ÆêcYî?l"ß»ÿ?|äЎ .Æ?Œ3À<¤)?ŠÏiÝ?ïC­˜˜×?".t»ss?ƒ!WÌñ9?l°ö¹wˆâ?•ÆÞep"?€ê)Ku@Á?ï9.÷S"?‡á§˜'?P²îÞ$M?PLMŒ×?—Îò'5Š7?‡Jbú¡n?ïÁÜRjŸË?´äÌk$§"?f¶oc	³?#–³ä}—?~ <
0ñä?´å[‡¤Ê[?ïÔg¼Å?n+‹ÅØ©/?Ttþ?PG(²†?pŒ_^\D?iDA‰ž`?¾h…û?uˆ5>Ê?r,@Œ¢d?\ºL
¨L%?€:Jg£ñ?s…hy®õ#?ïÛÎñ]®?dO5ºzy?.ȵTwÞÙ?!N0¸x7º?q"³ì{Á?c¥Û›˜‰'AGN3FGL J2220.3+2812@U°p@üÀ7ۚ?±Æ·À:†Tò ›ìÀ;Ëö³P$¿ê!È!õѱ@
SÙñÎd?ýU'Á(¿éð…ӿ݆³Äí°¿ÕjäJúm¿Ë²¹¹­AGNbcu?ïï0+ŽE ?a°ÇO㬳?#¸	Í³?ârRZq…?_(¨{mð?ajC½ßg?ï}ÛÌÞ¯<?†À~ttýö?n¶4Øp?o?æã5\?ˆé3"?'œçëÙ"?î×LË	Ô?ƒ|›ç9¦
?‡2ز¼´?pجLMƒ?™}\+Œç(?€@³orÅk?ï"¿؝?€Ù®g­¯?&àr?›u?2ŒûlÃY?ŽsÎNš&c?€ÊÛ\ëS?ï÷Ÿª?M"+˜âae?Þp®úC?§Mª-j?LÉ£+ݝ?Kv»g>!?ïׄìYì?lòàš¥[?TÏ!Šòn?RQ¾sΚá?nkCm?f…®Í'у?ïqSüpBL?rY#¶×*¾?{ni½/?fnùšïò?…óñŸ' ]?gæ.Û?ïèaÞl\u?Ub»n{?7gââŠ?ËWßÿ?fìf"Ýjó?TÌë‡ÎB$AGN3FGL J2221.6-5225@uE¸Ÿƒ¾fÀJ2ûÿÀ? À9`^SrmÜÀ;Ó~—µ"¿ü˜V¶E ñ@+óSIS0?þÒ^ß´[¿à+hjìÅ¿àŸÜo4É¿¿Ú«`êG¿ÜšÖœžAGNbll?ï´3£<ýÚ?z{cšL{'?O6¢"•ú?I»ž§Ï€?€ÿµ¡œÑ<?y`nù´—?ï‹ÛwNYï?ˆÖ‹vòùÓ?e'˜}îJÿ?s'æú°íÂ?‡¿<"÷v?ƒyʚŽ#S?îÆ~Ê?–ªŒY_ÚÁ?"Mœ‰ñ­m?€ÕQ+è?¥g¥Qnî±?'C¢6ä'8?îÚ<s<§j?•ñ6a܁?&³¾háO[?.ki%J¡Á?¢E…Tþö?•ç¨V‡€?ïÜY¤®m?pÄÙ$%N›?Bqâæß½?C{{Áâ(×?o	âËrtß?mÐ
PJó%?ïÙ­
î#<?m~Hº>äÇ?RÌ(t¬¼ï?R±³("i?lìàÓfÝ@?g,¬ˆkW?ïHJXWž¼?€ºn Ñ'"?'/ÓDo¢?m•±Â*=ˆ?‹Ú:"ڃ@?x
ƒ©?ﺌ"÷åÄ?r¾×e/ñ?q"Ò55"?äÃù»?GmC!­B?rU˜,˜ûAGN3FGL J2222.3-3500@#Lßàû®ÀL¨ñß«Ì¢À:ƒ¸:lãÀ<-*ÛuÝ¿ê‡Z'÷@Þ¬FD‡ï@ùã_`bÁ¿ãU¬žcË¿ßÕÖқT¿èÜÆè1W;¿ÖDf'§ûAGNfsrq?ïú î¼P?D\9±F¯?+žTÔZ+?2FVd?@ç‡çŽ?>¸Àa¸Ý?ï§èÆlOM?ˆ	ýÆ?bQÅ"šC?s+µ»»9?qˆxÊð?Á粓}?îË|Xý-y?ŽõŽn	¡S?ñv[n>6?…iÆ*6Ù]?•žþ"ì¬?'1"Ö°›?ïë ×)áÀ?az¿ð`œÃ?d^â¯?WpÈLü"?d•—S¸:?aa¢x5©Ú?ïýú%dW\?+WÜàÒ¸?àCj"±?Øu4eä?&mŠ 7O¾?%RëÐ{È%?ï⧈"Vu?iã?M#'—`£¥?PÄEúÜ?f"Pì4ÿ?cTïxÏƼ?ïƒ.29Ûe?y|z·º?~z";Ð×o?tO&?îRšâÝñ?jŸ\ÐCÇ?ïý#^ÔÌ¡?9Æ|Wwß>ÝgP'\ÖØ>ÛÙºß]^?6oj*ãiD?9ŠÜ<ìeAGN3FGL J2224.6-1122@I$­€k`ÀJì@/šøÀ9öÌP¦
ÁÀ;¾ðù²¿ÿ9H*¼@
±Q؏Ε@'ªo÷µ¿æ‰¡Ñv¿è³ifƒw¿Ò0ыšÊ¾¿ïùÓKþ'AGNbll?îTq»ügg?¯i)Æ?Bu?|˜˜Rrľ?†j\¼¯ÎX?§%Ñ3¯r?¬'*g2?ïQTèõ¥?'ùÌ1]?pï2|¥Õ)?sM™Ý?'™–dfú?Y¥«ñ?ëI=¨
?¥	øЁzM?±N¹°í?—ût:©8?´¥ª<?œ}ŽÏzÌÜ?î"Ð>ו? êª'oèc?P€Áî6ÓË?b'ùê¢UÂ?¦.öJҊ? à̌t½Î?ïB«<È÷ð?¨<¶®l(a?s´kT©Nê?€Ö™4²úÀ?'½}"úOF?¥šÐ
ÐÛ©?ïʚ¬Odþ?w<Öò_ï?[GÂ"Õ8?\6uˆœ_?sàægs±?r'­·»E?í"`Ðԙ?—‰­?¥ÀÛ/™©=?iô«ÝÎ?¡	$eìÂ+?‹ðŽxT?ï´Ù?ÌÊ?y[wõ'í?!ýDÛÇ}?"Ûõ̯Ía?'µ¥±²lˆ?yHӓ›iÝAGN3FGL J2225.8+6045@Z"O~ÃT~@wàmòÀ9܋Ëz½6À:ò
kùM^¿òÎ?`"Â@ŸÓŸÏ¾š?ÿ&´Nߌ?éÅŠ†`¿í 4é옿ҸŠ©³¿Ãê­ÈГ×OTHERspp?ìÆ+, ê=?ºÿm$?LîôkT"Q?NSb¿Þ?¹"ȱVœ?ºôtÜuâ/?ænžü"öI?ÔÀ¾J—™?–%­(d?š×âÉq=?ÑÀpÌ#+?ÓÁ†žôÍ?éìçTSr?®¤­Ñe?¥­ŽE·öû?—h݋¢?Âá¿à;?ªÜ9Gõ?í3,ÀRk?ªæ"&
? Å´¿Ó(?0˜ï)ôx?¶^7 ô.u?ªããË´!o?íýB¯c@¨?²Ç¡î~'¥?ET‹™t–ù?Hݜ‰[[?¯Ö'ßÁ?²¹â¾•kP?è·æÖÄ%?Ôúv:'BÕ?˜j¨Ç?¢Žy¸¥8ä?Ê™:µ?Ó~šç´?휀|š¸Ü?ŸõÙ?߯?"cP¦Cr²?‰ÛÊfw ?¬OßÃë?šSÙPPÀÜ?ï9	0Å?‹™ÑÞë™?[i¾Ha?7"ñN?œ'U'¶?‹‹¿Ë}AGN3FGL J2225.8-0454@M……rÀHj> N¿À8l'šÿÀ;g%ª´t?ñ2KÇ~¯3@F3´7€@Þl ¾4¿à>µÐ[øy¿æOEz³zk¿å€EØ|Xk¿êia1ëæAGNfsrq?ï²htªï$?ƒÎVòK~?y
'QCç¦?|tšÓ–?k}<í¢T†?lÄô.ò!?ìDéG=•?»{™=ÿ?¤lW¯"õ?¬#¿Ëþ?³‰ÿ˜ d?²¢ÎîoqÃ?í'@R¶?Ÿ|K/GN?¥l6'ºY?"§4ošØä?¡É@LQ?'òT>ó:?ç]	ÖmŠr?µøçÖë?·©Mݔ¬[?£×·|ýƒX?Æ·1¸'`É?³åw"'EŠ?ïîѶãξ?`
ò
ŽÄ<?WeÛ1'™¤?XïuUˆÒ?EínZ*Uþ?D'!â"æn?î"æ§Çã7? ‹ij?'I:+‰'? §œ9ý•?›9ðúoŽ?—š½çôÉÖ?ïl4Á
?Š˜Ž7Øã?'5i
³÷º?ù£o†J²?‰º é'Î?~ꥅ&P?ífI鋨?ž»³Î7Ö½?¦o8Û´^P?¾<ùöõ—?©Zbƒû3?—ä'Ò…<AGN3FGL J2227.8+0040@Pw[À6ãÀFמ_Ñ÷¯À9'|üªàêÀ;"},{‰
?ñ±«®o@6Óü–ê@'?ØÝý?äÒ»Þ+ޚ¿å©`ã<¿â¤ØXŠõV¿ëÎQ":èAGNbll?Þõùî)?Éûà?Ó9­*›	0?Æ奮Tí?̌»€°OÐ?ÀæÛIoé%?Û՛i
ÆÎ?ÇÕ=X>õ"?Ó%ÌáM@?Åԋy®?Ñ—µ¤ù/?¿°'?àn†Ã©©?µµå÷ŒP?ÖH7ÌÊô[?µççÓ¢ô?ÁµuWÅä¦?¤|u'²<?ÔÚl.ô¬‡?µýªœ¥?×Ç×R•VÇ?»…ºNÐ?Ó]¼}có?¸W¯+‹¥ä?äŠ5Í[+ä?ÆRB57Lü?ιï~ÂA?àÀ>ôÝb?¾:r—¢¢?²­yñÆ?äâ	ä˜?ŒÆ:PL¸?ʸ'R™Ú?Á"ìǜ"Ô?Á¿´­÷8?¶ŸêüÊ*?猛\šé.?®û8úî?ÈÐk8™_É?«ßá9[å?±úN¨¬ƒ?™€v8ê¢ä?âÓX Ç÷?±]ú¯ç—\?Ñ~¡&'öH?®®Œ:Ä?Áµ]D~µ?¦aWã¶bMIXED3FGL J2229.0+6114@Z© b
·@¡àE$¢À6,6*^x[À:tĪ¿[Ë@ž<ÓG:@'3DÐêi@&k×j¿Ø¼˜!I{Ê¿âêÚ»:¿åIÀÐó¬¿ì²Mx6{PSRPSR?5/íONÉ??øB"^3?ïà°Óá­É?sßÚZ¦Ø?l©.‰>¦Y?r¶ýÜOþÆ?'½HŒžÙ±?Ci5PÂõ?ìP=AÿÔ·?¹Lœš7˵?½r7LiÝa?¹DFiN€Ê?'¢I"^b?Ž†f$›B?ì"9	Oι?£¥õzF?¶½¥R	?¡^Š…ò¡1??j6K¶Íµ?E{Mà/ã?ï:i¤D©Ž?'µðM–œö?˜5"˜þ‹ƒ?'ƒù©ŒœT?3p CÆ~?<&Яþ?ïÊë'D¬F?…	R‡åÌ?ySj8?"³^}?FÿS&9'‹?aÜÓø´‹?ìkÙcDY2?®ˆ'÷n*
?¼s6>¼y?®aÌûŽ?§½q"á?©²4}ݒ?ëÒDLyïõ?§°õôÁæó?µYb$•ê?¢d»g/ö#?LBM;?A]Å$­—?ïI·GïÆ?ŽÙîðÏf?•éï[ ˜?Ç:ïcLPSR3FGL J2229.7-0833@KíàBËWÀIÛÒÀ+ԚÀ7¤ä+Ž#À;Hª9$
ü?ùÐÁÙ©ª@‹ÆùÏq@©x3îD¿ä'ë‹îz
¿çggWÒú¹¿é7dQ캿íàP8bÙ$AGNFSRQ?ïÁMKÑÿU?y_©/?xˆhróÑ?wýâbÙ?[CƒñÀ¿?T"°C?ïst1ç>ú?Œôý©Ÿ²I?oíit•­—?r}Œé˜?‹'™üR$?‡Ð>è°ô?îôß1ö•?å"ƒâí?¥e\æØ3?˜µ¸Ôµ]÷?"CYE?ŒŸlÀ"E§?ïRõ0vÉ?—s›"VÊÎ?rŽUXxc?|–… ºám?'q?•srU—h?ïÎæWZœ?tnt§dl?t…Ùˆ›ê2?sWDyj'?Pêï}]?H\±wäQ?ïÂ|—*S'?x÷Œ	'aê?aæ¸üva?`æJÁÆ?v7A(u[?sM]àÄ?î8l-$Ñ?žýã5½þ³?¤ ôôÞx?˜P+IVv‰?–w
^¹Úé?'Aí°ÿ?ïÙ@oÿ
ß?wSþòÉ<ž?\d5à'Ì~?i	½%Š]!?hu-…r'?rnÂÜ¡AGN3FGL J2230.5-7817@st­••ÀB8H˒:À9Eg™TÀ;¤`·Ð¼À«]¥wžG@ؗýZ¬@P_"äN¿ç óäq¿å`Hü.u¿ãL
2ïý¿ë[×ãðï†AGNbcu?ïóÇ#¯Kv?Sí¨Õn˜?C‹!²ùɕ?B`'¡p2?MXP\ZµV?OJÿ>µì?ï"ä"»?‹Å™º—9D?h
›#Ptß?'gj7KY¼?…"Óôî±?' ¼5–^?îÁvqA?´Â~	ë?'ä1zÝ?ƒ3©}ç?•OZZ?êçâ¡N0?ïВ@×-?€ ó_£j?"šñ«ä?5îa7{w?w†®qP¥?€'ÝPÊ;,?ïù¤Aú\Ž?B ÒN>?9•ÆeÞ>?5-X©,?9@X¥l??4ºÄ"Z:?ïہ¢ˆ?pd3CîÔ?Q²âê3?Oö]m?k¥ãÈʆ7?k¡{–s|S?ïgφOZ?€yUKÌà+?…'‰ý]õ?|T'`øV~?€‰•?ﻄ?imE•êc?ï÷™ã|¢Ï?UÔ%À->"ÄA;èþ>­ƒ`aÞ°&?PÊü×nHØ?UÓ©ÌË×ÑAGN3FGL J2230.6-4419@v³¿µÀLƒT_Ó¥.À:P/žS<¾À<V	!ò¿ã™õ&­ƒ@
ŽYõiÏ@"NàbÖº¿äÌRخǿèq‡DÓ¿Û9'Åö"¿í›oËÑ
…AGNfsrq?ïàãeüšV?k_é tҀ?Wґ°µ ¦?TZ8Ŗ:%?c3QLl?eÞ¿¼¹œS?ïHi~|e_?"ç"óCc?v +<Æd;?";J&¿Z?'jÅ\Q?Žˆ"jÕ®?íEhâ9?›JO.'bé?¤±DÛ)y?wé=Q‰?¦ø-ÆQf?"#Âór7‡?îÄAD\À?–6™
¾?k؊0H.Ü?oSœ|{eL?¡þcûŸ0?"¬h'¸v?ïçÅÜ,e?_üE¹L¯?W'çZ6=?T>¶Sš$?Xá`^5Ԝ?T[jƒ^?ïƽϷko?uPÖq8>ò?`(ÃҞ?]Cz=ê?tŒ¶©???oÕÖ:¿›?î˜ñoˆ<ê?‹Ÿ9êÓ
8?šM
HÊJ?ƒ+ZÔéM?'"ÄÃtü…?~\PxC?ïÆ얟Fà?o@Öè
<-?P,Ñ1!ƒ?DÝ40þښ?x~°V>æô?lÚÛáóAGN3FGL J2232.5+1143@SZÀ5¯åÀCJ—à[õÊÀ7X‹÷§qÀ;#¾Šêª-?ü«zŒãþ˜@"HM÷"±@·'TU흿ãv-¨Ò*¿ç·@+T¿é¥*LbaÓ¿è‹隸ÓAGNFSRQ?ïëPs5é?`‡DXzºŽ?Ux¶ü}'í?Yh|OG'?SæbZH7?MšÛŸhb?ï‡×füë?:†ãÑ¥?hózŸ"+Ž?zÕ/ðµv?‡ÍG"^ä^?"£ÆäÃs?î|ö玫:?ù»~»?•îDLÓ?'±Çéì¡?šÒ%
µÞ?•DûîXŠ?ïÝUWd.Â?x»¶n£a?0.Ž¨e‰?OÀ¤C©ý?pRk`äÚÕ?xymiæÔ°?ï󏭘»4?U¿`B'õ?J,·~pÍí?IÞVŒ	7ò?G""Åòª?H¨j¯ð´?ïÙ¬[æõ?máDvÝô?Rè½g­Ïä?R@^¯çÒ?lߎóÒ¯?g%\%²Ñ€?î·ì(îÇÛ?—«ÚÎhy?"Ȭ_LŸI?ÙÑñcã?"9΄'3d?'2å˜f6í?ïú¥)3™Ï?Qf4vb7?Ý,áÏ?+ôh¾à(š?Aﺜ€&ÿ?P"E3÷j@AGN3FGL J2232.9-2021@Bºø_øŽÀLÙÌÿøsDÀ:A±Y©¿'À;ϳt62ÂÀG-BÖ¿@×3#žì@¥ùÿŠå!?Ç%£ø%M¿èFz™Šf\¿Ò_½m'Üj¿å+ñSAGNbcu?ïéõ³\ ?aÜ	—¸?1½¹z}÷T?0x=v³ck?cҕy§se?`vq"Ó=?ï™i±R%š?Š¦lwÚ{?f9%±,—¿?{î?€Îèu?"J1Äù?3ÔDò—œ?î^qØèír?XÿJ£gN?ŽwñºS3À?|4|üÛSg?¢zæK÷å?‰þ
Ú<ˆ?îím2LGE?–ÎŒO
'—?"Ôô¬Ï?2½*d1†[?¡
ØÌ?–ÉÔÂ1	Û?ïóZÁ¨½Š?X]iÏãù?.A-|VÇ?=z±r?U‡4çd9þ?S·Å`h;Ñ?ïÜVn»c]?n0v@F9?Q?¾:D•Í?Q¬ü-P°É?k	²$º¨h?g³-5匄?ïKrÜ/Z$?}òûÚE?ÑÍLÚ?p"Äë?ö-?ŒÇu?u¶´†~º"?ïÃ7ÐÚV+?r¨æB†Ž­>üôÌ®?Ú º2?~G÷¦ÅE'?r¢a›#ÓAGN3FGL J2233.5-1235@I&û?¦ÞüÀKR·?œÎÀ:N(´T0À;µŠª¡¿ü@Hð^Í@z}[‹a@û!_Ìr¿æk½à˜(¿à>Ó	Y)¿âR~WsÚB¿ãº#r AGNbcu?ï䄱L‹?gKRnP¯?C1pÈPêÙ?C·wIZ?f®ò^¾9ª?eÎÀêVА?ï›	"!Ë?……!jócÆ?bÍq'¬Œ¦?f2MΠ§¢?"Š>òSûó?'V »ß,?î³"–?"õ¯",ÍP?–nø®C?…:à¨V2Ø?£MK±[§?ŒÀÄ­xÜ{?ï`,XN?…<'?Êk*?*ÁÑô'é?-K¡wó¶ë?"ºŠy÷{?…(Å,½?ï÷ÛT½x?FÐZÍãA"?,çïL©?-ZLa?Iˆ2£Ê*?D#p7$/ú?ïßnL[DÂ?jIrú>?OãwÆL‹b?Q3w#œ?h˜ÕŠœ·Â?cvÒ¯›?ïU4ã•ß?{ÿ7¹î?$š<ç?k"bábºA?‰Ž-ÅÝ\?tYdù;"'?ïÝ9à<õ?_؆‹Kì?P‹›ëy?N͑sÈ?q8Üé›&Ç?_¨6Mð|îAGN3FGL J2234.1-2655@9N¡¿ØȄÀMÂ'?ßéàÀ:êÛ«ŒáÀ;é"C÷¦•¿¸cðHà–@,¶Á™®@ÿ²}@¿è ‰	Ôj%¿à'<\kš¿äžª|.¾s¿×À<­Ò®AGNbcu?ï÷piÄ?Gº?À2à?7EšYLa?4GH¬tä?H`3?Bá»t?ï"rÑçf?‡	雌#j?cKúJІ?e?TÉAè,?†M7èºï?ƒùÝYÀnM?îÝʗØ??žÕDtáð?ŠòGƒíÍÞ?zá-v?«F?–͉:oË<?…\ð*{ÒÕ?ïXfüìع?ˆTªý™?P¯%ôGn?PwÚvã•?"è/ÙÖXc?ˆmƒ$Þ?ïû«"eI¨?:I¹lsð?&ÉPÿ¾?'ÉPzU;?7¢ù	97?2°ˆÜ_.þ?ïÝfd&ßØ?kef+ñ?P 
²¶B<?PN5n³Ûý?jI•¢ÿD?eíD9áeE?ïˆþ"ˆn?t­–¹i?z˜Ÿ"ÑFÀ?lAîê[a{?€tU²†?jhx¬:ŽM?ïã›jvÈ?`«Æ$	)?8_dêed?,q
pͦ?iX¨ä–g=?_ãz´·7PAGN3FGL J2234.8+0945@S "AÀD8G@0q¸À9"h¸P>À;ž
§ù®­?ú$ÉñP9Ô@ü¼(º´F?û¶\/Ö²T¿¿aÊ®Q¿Øý˜MY¿ç]RÑÅ@¿íò'³e6PSRPSR?›pî"B£±?›g°Çº?îä•I‹
?¡3¨lþØ?ñ¡!1*Ö?"N»"Ô³?ËϞ½‰§£?Å-hæ?ÜÜ?ß÷2Ú{j?ËC×e'å?Ó9n`°Å?ÁÉøІÎ?¶T‹É¿œ?¢¾	°?éÉ?꒾Žúþ?©Ötÿu´?µ¿¹úô?É†Î6?Ð^€±ô·Ö?¬Æ6j&8?ãºû15?³U›÷܉È?Âø¯ÉË?¯¢¯røø?¦Ud¬ð	?¦ø…•ß-€?îg˜,ÝÐ?¨†q}(œB?yˆÄJJc•?{è
äâ!±?×4LQ¬÷?ÉÎáÒøc?ܺƒú~"?Êt?>?È#NT²ðê?´ál"'s©?Ð0àš˜?±ëANcl?塦éþj?²Ç23oH?²/Nߏ†Á?™A˜ñè?ޕeOîˆg?­/]ÍôÝ?ÝA,¥Ð^¨?¬S¨)Ç}?°¥¸%"ÇÊ?˜x¬©‹MIXED3FGL J2235.3-4835@u‡É¥ÒÀL1@ìFÀ9?ÿxÃÑÀ;Ï3ÿáÍ?å©1°¸UX@·VƒÁ@æÄÀ8ê­¿áø4Tª°¿æp)Ý'¿ç­;)¡¹ú¿ïÿ§U¢|uAGNfsrq?ïø÷бˆÏ?Opîó)rÇ?,…1eÀ¢?-×ÚËð»?Dü›ßÄå~?J|Üõ»æ?îZJ2önÔ?¢6…©í¡?XH¢xhÜ?có´1Z?£J¬F{'?œó%F΀?îÞ`ºø0u?ˆa'\²²?"¬˜ÌU‰?¥CµN8m?FxÊӜ?yÁa‡K?í&€Ýµþ)?§'µ˜1÷?¢d-óu†?˜oùä½AZ?«3Ä3¾Kê?¢†LU-™?ïúÁ²gpÒ?grœÀ˜Ÿ?0'mtó?R¸d¼x?9`þœ½Ó¶?\jðgõE\?ïG½¥¬;L?ÛH"¤2?€ñl3ÅØN?}	Ì."´C?*g²–Á?"ø¸¿rÉ?ïFWã@׌?zîEoχ?ŒYF°M2?s¦ˆ¥‹\?'ÀnNû?ls$åE?ïR@'þ[ ?‰Hv+¶?"…!@F?rHÌÛ7	1?†ê¹òªô?…dS®×-AGN3FGL J2235.6-2319@@.Vßà¥ÈÀM"
Ÿ–2ÝÀ9¥aÈqô9À;ÒaCöÈ?êô³JF†@ÐÎäÿô@‰¯ÀL‹Ê¿æÁd»ã½Ì¿ìm<<'x|¿ã@`óaK¿ï¯òuÝ
AGNbcu?ïö N —?Q/`õŸ
&?85úŽ'»T?@{jáÕº?KhF{W?Iýšâ3O?î£Fhf")?¡7…ÛÕ1?‡I~›k?ˆy5΂á?Ÿò¥·O±?š"ù 
9#?î$Õba?˜ï$H[Nà?œ¯‰M¤¬%?ŠÆåN›;?žÎ4?k³?'ÊŒÿÍî?íTE³N²§?¦¬Kb¦?™iÏÒe½õ?¯ïÅ!?®¼ã™Ä—?¢:¸n¹?ï÷Z
"äm?M/zëX-é?=šÄ.F# ?>I®':Ø?CÊiÌäñ\?A¯¥G"µ¶?ï`P¹Å¢Ñ?ŒÝû Ü¿??} ¦âƒ—?{uˆBJä?‰~$Œëû?étd·'à?îÖ"ý8­ú?'aՒ"?'›)óŒ?ƒ1ç	`:K?",—Á/é/?‹€p0bË?ï?®‹]0?"tè§ä€?Š‹×C†-$?rºåã)ö–?…ˆ…RÃNý?~'‹R­AGN3FGL J2236.0-3629@	tŸå
5ÀMöWŸúëÀ9lÙÑ.[À;Âßp=½?ܸA_r@á!c|ý@›ú¿Ï8b¿Û™`GØ«¿äø—'=J}¿ãêĊð¿¿ã4dœÈßAGNbll?ïú¡[9Ñ?: $£
¨?¬éÆ@`T?¸1 ›±µ?Båùß¡†
?8–r˜îqq?ï|b'$
?Š·pîJc
?iœ‡TYˆÜ?k"–pÐè²?Š€9¨¨÷?‡
~8'7?ïC
4¶?"4Å è"?"}q
ìú*?q_ú{ےh?'ÿËæA?þ¶µ™N?îěò¨Î?•¦Ç£™×ë?lú9(Ø?fŠ»þb?¡ìo{ú&–?"ØßïX+Õ?ïý7z×À?+t·VRÐè?–mhÿ
>?á Æ8þã?1"_è}•?'(ú'$£?ï×l)±É?q˜×—¡?T"¬Â+¹5?SJ~÷Rl"?nIÿå=Zù?k@‰¦"k?ý¼¦0?}\ɏïŒk?u%û֒V?pX!9k'?™m#˜¼?xâ떕Cü?ï¿Ï$"³r?t'­­=ú?YëتøMñ?H
Wÿó?yw­;9?sAeøɖAGN3FGL J2236.0-1706@EÌ)ÿ­Ê©ÀLšŒ 4RîÀ:N×úþ8€À;ÓÂ¥+ž¿ôsÎq»@@å""@
3 "ÉK¿á™»&ÿj¦¿ÕTR|¿äÖǪ¿à"²k;|AGNfsrq?ï÷oª ¿,?B뼊¿ÓÉ?4Udߐ÷?0Ú¿³??H¤o²Þv?>šäq¼'ð?kP8°?‰	v€¢Ã?dÇÔÝ؅?sÊÓç]ó¬?…j·SÔ?ƒ@(±qt?îÍr8¤Ì?ˆ¥œópn‹?Ž­KDzlþ?|Û	|Î?–ûIBp?€˜Ú¹íʐ?ïtªsv,?'ûޏÅ=ã?7ޑÑûѪ?9 Pþäž?'7Nrj0?'Ôb€óAk?ïûjçKöp?8Qô—&°?"y¶ -H¨?ß}†Ö"x?;këaý ?4)g!ѕ/?ïádÿ‰¯?g°nŸ©SÐ?MfEtª.ï?N7!@¨û?gAnü_Q?biqˆ®dØ?ï{ÿtŒ;Z?sلêU¶Ð?~¹ôé¦?kÙ%¦zÏ?£•Y5«Ô?ed>#jS?ïãÞ°5M¦?[·¬
Ï	?@ºÏ•?©!¯oíc?k‡OV2ÉL?[o
(Ò%AGN3FGL J2236.2-5049@uNß°Õ ÀK"î²ÑÀ:,M…>À;ã"q;¬~?֊Ø*ùÓÁ@
'ÇÍ3¤ó@ÚP (êZ¿áéÒ­˜¾¿æÜì/œ-{¿ëïée¿ïÿÝbh¢MAGNbcu?îæÄÙtŒ*?¦ÊX·ÓË­?dånŠÉ[w?gìƒ@"Å? E[²±¦?¦R®ÑU?茅OñÁ	?ÂÈCa(m?»,æ%?µß:œ¢ÒA?À7é»ÅéY?·hHËå‹?êä¤4¬?¨âœ/¬5?°á¿íu¢?˜dÆ;(Ä?·ùÎÎßÀ}?¤";)Îdå?âcò¾Nï?·	UVÆ »?Ð!GŸ0v?·Íõ´h '?Æ-¥È¯X?¯`Ñu)×þ?ïO	lݛI?œÑ—øØå?dì[†¯K?…*žßƒÓ?"FúUë?™ò]+ßiÎ?í¥8éÖré?­^`…í8?¢I]Ÿ ø;?£ò-èó(i?£c¿ˆ=<?›Ì¢gx©?í7Ìs` ?ž³ŽA´›Í?¦z¬2gJ+?'ƒ3)6Õá?¦
7yÖ?"?ðøÿo\?ëîŽ"9ˆ.? mÇàF*?²°
Ç1Áê?˜?¹ñKÀ?«·RO|A?•ëмk÷AGN3FGL J2236.3+2829@V†à€øÀ9¢¬_nû`À7ÛAõmÕÆÀ;.ì³òá4?ø¤Z­ Œ¨@Çj²ÑN@5¸ÜU
¿à-Îy—'ü¿ãbºFÊ¿æ·£®à¿èæÜ­ë`6AGNbll?ïãâèíêª?béŒ"|?V"àdì­?XsKϙ?`Ó†f#?XøžÚ°m?iQRX?'h~eØÔ?mþÝ¢'G?vª¹Fœ?ˆ_Þ'Œ7¼?Œo†BX5?í¶X#ÇI?¡>ø"n,?¦ÉÁ'ó§?šïY2®ûl?€g€?'t°$Úì?ïÆY³-G?	/¶÷Wv?@lˆ Rpû?HÙº'ï,?zìB=ÿd?€áa0W–?ïïi:3á?XK–e4r°?SÔBIúi?S3>:23ä?J³Á(ô@?CÓwÛCB¿?ïÐo%‰t?sï¾Ò(Ð[?YíÉÔð;Î?XZr>mB]?qM}~—?n{"rµ?î½Ñ»ãµ5?"÷èx\¯š?™;tÐU{.?'ªê•XÄ?Ž§fg¼H?‡WÔâ¡ÉŠ?ïôvb:R?_¡øNä÷1?3~"&¡Æ?6Q;•önò?RL\ʤN?^5¥p•ÓâAGN3FGL J2236.5-1432@Gñû`^©ÀLßùÐ;À7y#zX‹²À:ÓÔÄ(?ø9ÕÙ滶@ VĹÜZ@#Ì:«¢†¿Û3T
ÑØX¿âQâǓ†¿äZÀþd,¿äØq*\yAGNBLL?ïð§ìSáæ?WÔs=ô/?0*Gã‰{–?.æð–
-?Z¥•žè¹?Uæ£ô¢ô?ï¦mëž|¶?" "õf¬¯?aEdŽÎþ?d^€·øÎ?'+ýôõ?€öePãV?îlïÆr¯?˜ï‹Ã·:?©ãÈú ¿?ˆO‹'Î? Üï"ª?"DRÚ`?ïúPŽ7æ¡?QÆêíö>ِƟ*þF?t9™¨à?FŠ¥E^2µ?Q¾¥Òjü?ïùÚ_eð?@ä,ÿ'Ûk?$Æ+îÿPO?!7rqŠ?Cd÷Jóg?<çq"ýþ?ïâa4"q?iTL¶!?M2A†¤?Oo‰ƒ?f4`ÿò?bÂԏ²³?ï2Ë¿ån?Œ¿wìÏ
e?"6h°bE?|Êu³L$q?FÙ§Rt)?†tŸí¤;?ïÿ³Õ?.e2Bä¢>͆@áUÝ>ôèHüÅr?ñöÅt3ô?.+'0¨AGN3FGL J2237.1-3921?âôÕ@"ÀMÌÿ ^¯¹À9§×ÂÊŒÀ;Íiϧr ¿ÙêÍ×lk—@APt6³›@ßß»<¿âCq"öO[¿äF†TËè¿ãèN.Ð稿á@ëæÿ(AGNfsrq?ïûIvãÙ{?9h¿ÊÏû?ú^ö+?]µ»Ïú?Aƒùo#A?89®Hν?ï¯øJvh4?ƒ//ÿp?^$R%)ðÀ?c't© ¨s?€=c'¦ö?^;s@bõ?ï5©tzr¯?"žyËó‡?€†Øäì?j£ÕõLî$?'ejŒ¦?zˆ^Nc?ï쬞·™?cÞNh•¥>ø,€y,¦ñ?ôÊb×Ö/?cÀúid³ä?cÏæ|=?ïýêø˜í?)à vÜÍÍ?ø¼Îq§÷?"o?$	+?+'K*¾ès?'CŸ=äHò?ïã[º:ùÑ?h²÷##?L"s64S?Okä«-^¯?e(Ô}±?bk'AÊe?ï®°#¹;?iînD—à?oâiã¼²?`
Q4˜"€?x¶¹fÝÏ?a_§S@AØ?ïý$ŸWÚÄ?85ðZ!/å>áh—–´¾>å¤å–Ì?6OÀŸ§Vš?8ËÄn&AGN3FGL J2238.4+5903@Z£h@[9â?ޝ¢ŸŸ›À7±E‡ÉÀ:²›ÉÂ@3¢x:yN@Wúÿ'?þsÆV;¿Ñ–·÷þ~Ì¿ãÈ´˜p¿çìÝÖVÛ¦¿ì›R[ÂsƒPSRPSR?<Ô60vÑ?7~RCÆS?ìk¡'ü
l?»b›­¯È?¼†ì"y…c?»XˆÛäË?[;÷ÛvçF?}>Ôwù"L?äÖâ˜n©ß?Á­ì /h?Ö6þ×}*?Á"–g,`?…n¬¤Ù?€oÓÍr?èaÚ¼V?¶bíWsê?Í!ªP1Vö?µúëFŸ›?‹ÕLÅwæ8?'zR3Úõ?åçnsG—¼?»¯ä"˜ ?ÓRx³EW?»/¬ôrâ?+ru†…u?.•,&ø8?íYmÕן?ºDb´ÄÝ?µ)kíÑ5?º>)Jž?pšH*8%G?~šÐšôwá?ç`Nõº	"?´.?uð?Ðüøó‹c?´ŽéshÛË?†_Yȗ`?†&•
ì?éå÷´?²²(fé}Ž?Ê:vN÷ðù?²Jƒy:S?‹Ó
19ç?€Ó=Ák@?éˆWý9sŒ?«äÂý_›?È-²Úw3?ªý.BÍHâPSR3FGL J2240.9+5831@Z¥ƒÑF¿Â8ßowîÀ9•ÝŒ7±GÀ9›V	÷Ї?ú±¯ÀL‹Ê@¼%†¢F?ìêŒèé}¿Ïà'·)ø?»Za»¿ç	'6½›¿ïÿö¯Á›ŽPSRPSR?m³ÓŽS\?‡±})æ?µf#2¬1?½âŠl]©Ý?í6æ%õn?¾‰FvZƒ?Â-ÔÉ	b™?ÎAZÄ­Õ¢?ÅoÞê܂L?Àx²íZ?æ"†Ç?ÏÒ¬	Þ¦?¦×i š ?™ǟåƒÀ?àÿ^ƒ5)?´Ô¬µç?Û&V¸ÀȪ?´}ÔmrL¸?¸|Íd…Z?Á"(âÞm?ÁpmÑ>Ì?Â]À«èaå?萊7B?̘zѓ—2?C@p5éº?rþ˜è<ìz? 1£6â{q?´½³
v)?îøË÷ÃN?´·!ÜÍ?ÈU¼?ÐƜd­²?ʔaê^`¼?ÀzÜ.Œ?ãE¤–f£?Ϊȴûù?±0ô!	ý?Ÿêúžçî.?àò偾Jm?´yû»ïý ?ÙÍ÷ô\¢‡?´*q×S{?®¯Šƒ|?½§'¥û¤?Ç@OKÄO?½Öy­ŒQ?èDóE÷õ?ÇJýtŠk~MIXED3FGL J2240.9+4121@X‰}ßÿ¯xÀ.Oç_JHÀ:¿k»9ýÀ;|Î>½¿»x'b@敠¼@ž2 f<u¿ã\ûn¿ëT™¡ô~d¿Ôû¤åìÈ/¿á.»c\µ|AGNbll?ï͆á[$>?xìA1ã? dÞ½?Z?Ï=3˜#<?x¹hBèX?x·"üi?ï!Ñ3íJú?œ$м<ÿ?x¡wW§8?x†žñA~?•{²p-¤?˜ç©>t§>?îü¿?–(ˆnÕÉì?FàŒ°?xx<cEè?§æ{‰3&?"utæ¦?íIÐßè¿? ÛÁ@ފ?`=$Ö%Ÿx?`ӿغ?µ/ÚÓö? ½. ="?ïìþߪ±*?_ܑ .`?Øs2|Ç?Юöy?b*\«ïµð?^e°£b·?ï»2E¢v?"à!]?`¹Ö¿Ð÷?]4XÚߐ?z
Z,y(?zð¨ËÅù?ïJN¿øöC?~m‹2s{À?|k¯œ×cï?g–(±´o?6x.‡IW?{{¾â³O?ïPÉ|òU.?y2c\u;¶?]5Uûö¸?JQ‡åa?"½	=ôá?x_-žÞüÊAGN3FGL J2241.6-5237@u®6	ÀKuJÞ™À82ª§ÞÖ»À;ný`O@N\Õn@jt#"X?ü‰ïµ…'¿Ð©RÝ{#j¿Ö¦˜"Š'"¿âÚ°E‹-#¿î¸R‰åœ|PSRPSR?"¿i"À²O?†ræ›bÄ?%c¥?Œ†.W×,w?kg4ЕÑÝ?o.?òËòW?–+Dµ
SÖ?±C†÷î¸?ë›.šK?ÆcŽôé»4?ÀÌ*®‡ðØ?ÂP'Š†¬?§­»-û?R9Ã!&?ì)RÇx$)?©FV–-·?²ÞÛèg•¸?¢¼æœHùÙ?™Ç—csÈ?´\[—ù?ídá=OÊ?¤ÆÇ:–É?¬Ûv=0þt? h*¼»3}?FŽÛŽ}?H^?ïp43Ên	?²°®Æ?"Oã@wVˆ?±X­;!?£ºxËé"?·"¼«"Á?ëA¬Xõ ?Ç{ûŒ[v&?½–bŠ0=?½‰TN·?³¯Ÿ¾—m?¢¦á³þd?ëJüȼ?¬ÕéTbšä?²‹p9œ®?¤kŒÆ†?ª54Û£?"B2.ÅH?íN«Í)?›¿ói|lù?¡aÁ_2?º|Èez|PSR3FGL J2243.2-3933@vyÏÏÃøÀNW³ S\žÀ:eÄ¿¸TÀ;ð^VÀë~ù°/³@/B%¿W@ò«]ä¿ç—™‡jÿ¿ÝÆLM" ¿è¨šSd¿çj3;°tAGNbcu?ïÚù8™,??eèˆE°w¥?XUaÁ?W£‡GÂï?hÜs	d?_õ«ÿ$öH?ï}ÕG¼úi?˜ä癓?m?œg$Á?'ß°EÖm?‰:Æôrb†?'¢­Qwæ?î{C/Í?'h†ÞZ˜?—Ý9|YŠ?ƒT+Ñï?¤'_ÿê½k?‹j‡G}K?ï(¸,E?œ4|8©¢?@·—.oº?QÇ-Ž$±?šc=¶¸ü?œq¬ŽÀù?ï_ɝ?U+q‰Œ[›?Bތsð?>ø´×.N?Y;sAË­?QNêâÍM?ïÜísWÝÚ?qߗ+íV?R<ØÝÙí?[·Cäá_?iô÷= ?iAڗòï±?ï*;ãät?7»mÕÌ ?‡`Ƨ4Zý?sGdÆÿ?Ž@mm±?t{$®të?ïÕ1'z^?wVmma>ûù–&rM8?^LÀ?uK>)JŸ?wœ—WAGN3FGL J2243.4-2541@<t/ ~û‰ÀN±W€•ÓÀ8¨Xçø¢>À;'Ì؋Fð?æƞ‰\Ny@ö˜Ô!Õ¾@2¹@(<¿á²Í¯m7Þ¿ãV'^o¿ä~v"T#¿ê‰2°Î¶ÔAGNbll?íÈv눓?ÅDË®a?²i©ÄR?Å.ƧnÄY?p%*m¹?p3Òè2??ë+UU
ã"?Á%íX?ò?®ãðVr`?²@%!1/?·3]Lý­Â?µw|CøqN?ëó¢Ý÷'Ð?¨u#(H=?¶Nþ>"?¤¼A³¥£?¤'Õ"…Ñ?Ýšö¾?åä(¡‰Ó?¸ì#D^Æã?»ÿ‡'Y¾Á?«ýD]ÙÎ3?ÊoóËòºÑ?µ&í4äGÅ?íe‹I—0?Ϫ¥
|Q?´cL$?ϸ"Ú½Ñ1?\B¿­?aO†s½[?î*¹>ÐuN?§]eck'?š€s>!_?šg|Í? 2px_¤?™Ü8Böü?îÑônÒE³?"Mbò.)`?™A¼ Ë5J?' (è¢-v?ˆÿjÿ‰TÖ?|ÿí&,¼+?ì˜fÍ$ǜ?¡bÕÈþ@?¥DU"¢Ú?'æ"Û/4M?°šÅíÏ?³?žD°¶AGN3FGL J2243.6-1230@JRe?õ¹UÀL]â?û˜'À:%©|e¬,À;ÁÔ2Ûÿ?Ö®ãû	£@p-è±@ÀÊ+¿äG.B¼Ö¿ì¤"{ó¿¸Pí ‡èu¿ÖãlØ׃AGNbll?ïåSUVb|?g¹eg:O?nl"¤¨?ÃëÔç¢?iù7;ç?gygzێí?ï‡Ër1˜?'h'3Є@?füš™¤Ý?uû²D¶•_?ˆN}.°Á?Š
¾b.{ò?î«]ÍvÒ?Œ*^+&?†3¦‹ÍÃ?s§ä[³?ŸzsMOu%?‡]Šùƒð?îK9o"À?œe¾î	Tà?TcúíƾR?\NVÔ:èÔ?ª«Œ'Aˆ?œ?šT•£?ïôȽ|?O֗Uî8%?/
h'ÿ_?ß×ÂZ³!?U<ðÎ2¾?Nô…9‡óß?ïÚ»F´è?mãÏÏ®7?S‡p¥™'?Q ÉԕÞ?lp÷½?gòÄz6f?ïpyV?u·Í3"tô?vã«q©?c}E%Ó?ˆmËãØQò?r!Äå:?ïªñHŠ»ä?see±žì¿?SñoaC?OñA'¤†?'Åð]ó?r€…Ùk¿2AGN3FGL J2243.9+2021@U¥Â # –À@®(€QÉ÷À7³ŠÁéÀ:žoStò?òý>áß.@QŠDg
*?ü¢Ù;(ö¿Ö"÷ïÃÐW¿Ö'ÇɾᎿÙüÚkÆ̈́¿Õ¢/ÁIòùAGNbll?í…÷+M¿.?«1EBY?›Þˇ:aõ?•¨^¼–Î?©±'Š'?¥*¶Í;p?í…›GLM?¼êN_UóI?˜jçKå?­‡õ³À?«z:UQÆ:?³€¯…ò¦Y?åQ0»£s|?µ]»Â\ˆ?³3ÕÁ#\?ŸR_oèui?А©pAå?³€Æ¦ýa=?Ü9¥	±§?·Bõ£#¾É?¨ÒS8P^?¢q:Aÿ°£?àg½ùö%·?¸
–]¯E™?ïé.àƲ?™NÙÕì?Ž1¨†«Ý?ˆm8ëîuö?Šä×'?¬³yUµ?îŽBƒ2O?¹ÑØp2?'ÖÕí»bu?ªR¾‡È?œ`Ù¥" ?²
8'€?éÓÊh!/-?¯rÉÊY˜?¬ÿ,aÜÂ?›rˆÞ ?ÁqG©.Y?ª$¥uÌ´?ã÷ø¿;a!?±n¢|ō
?¯êӗóû[?–å‡=Ro.?Ô´
ÊT3?±lá.ŒÂMIXED3FGL J2244.1+4057@XŸ£ÌhúÀ/"yÞé/À8¤zôŒÀ;?ÜìՁ?êÛBG'þ´@ë¸x¬äû@POŸ¥wH¿Ö¹k:p¿åT|/6µ…¿ã¶C¦üaC¿å'|/Œ›ÀAGNbll?ïúbúºà?>ëšš}?4õ¬mÙùH?3aÝèÃkW?:ï<÷Ug?1£Ï4©}"?ïyÈ
å
?ŒºS.˜r<?nÙY>â ?qr&ÿ]?ŠÉÞÿÖð?‰)caàUý?î»–t\Z?›Jìì?"ùÑ]mRñ?‡kjš>?"–;Õ¾ïÝ?ÜaÑ¿mn?ï›vS€Õ?'¾|ìQ"Ò?AJOpC"(?Açø4ÅRÕ?ˆ
Æ5Zµ?'"÷Y@uª?ïý
®@?*ß|¤yëK?&t‰ô ²µ? )ÑnZ?(à"fg/À?ôsÈ?ïËȇ\™ù?x(²^P?[jž½?\TVš´ñ?sX¶}: ]?rônRÌ1C?ïfб³Á¹?|0¸éšÖ?ƒ3N"
H?y˜ßF¹X??ƒ…Æøu?u/et¬*è?ïꑔpž?`m°Ñ|[‡?6ŸžÂvËo?0÷j#ò÷?bšw·ßçD?_'¢Òñˆ¨AGN3FGL J2246.2+1547@Túâ€'،ÀBµâ (zÀ9•9"†À;<L$ˑ?çgØx@rP@Ùå_jÉ¢@v9à¡jô¿çy¯nm¿èû#½/²¿Ü'øª˜'Ô¿Í&hä3àqAGNbcu?ïòÜÀl?bKàJýX?0±Q·+§`?1Å-=?W§óÜ~™*?ap‡mÅDá?mvê²?"wÉÆ;6?hfDëá?hzúѦ©?‡}SXeÉh?Dléÿ·Ø?ïÚGgPO?Š‡÷rÍ.?þÛ¢†‡Ù?pwþÓ?•åIEnI4?†ÛW[ýS?í‹FI‡ÕÄ?£GxÙhc,?`¿8úÇUÅ?ge™cžý?³ÓêTEr?£¸•Ë=?ïøiöÙw?Y²ÖߦÀ]?-º¶X
È?=⧽ñ÷?FíVðÉ?Sæ<¡Ò;a?ïÖb:áñ?pgþ
Ûäƒ?S°Aø›?Q(?\´Ó[?oÅ¥iC)?k~fF2ÏÃ?ï¦>ø?s…ZB?pcj°£v?az>d[ ˜?|Žwƒ ›?pZ2&öëV?ïWw-3ÿ?ƒeÙ<3š\?`'´¹ÿ?d?]Uno}?"ü†BJ?'\öÇ]§AGN3FGL J2246.7-5205@uFŸŒ!âÀKí: þ¡À:-¼ÎRÀ;ƒìŒ…´à¿Üœ²
™@
½Úg•œ?÷!ÀD(N?ïñA2œ¬Á¿Ý+$Ÿ$P ¿Õ~uh"EA¿³ÔꎺԎAGNbcu?ïBÐ4³f?¥ú}‡:?0aëÜ.ë"?3=58"áì?—dx0°zp?¥÷Âmi?ï—"Þý&?‹PÊÙé§	?e´-ÜmH?|Žp¶?"Ñ+ö
Û<?çñ§0àº?îYUB–lW?"ØÁ]éüD?•"ìvqˆ?‹½4àN¸4?Ÿ³=Åãm†?‹¯ß5˜å?î(W
Ç­˜?Ÿ"îÄ"Â?8Ùd¦˜éš?Aà{†ƒDG?­HÜ]{•©?Ÿõ¼SY¤?ïxsjl?»%A‹™.?*–Û»#7?-åÇejR?ŸŃWbè?»\E¦'r?ïÝI^e2?l}¥KlM¦?PV	8ûk?PЗ*Ö!È?j‹œùÆæ?fÀâþ¦Zf?îôÛÅ?"žJêp1ý?µ»âd|?ŒÂÀs;ûž?'Rçh
~ª?‡A«Iƒý\?Gf?z—¨.Y?)ì6•ýžÅ?$8É)nàþ?‹'ÌBZºÙ?zÃps€¹AGN3FGL J2247.8+4413@Y-÷ µíÀ*€Ô`?ùÀ9¾P"–JZÀ;}ð·Ž?Ö$8'¨T@ "=¼Îþ?üºÊÿm3	¿ä‰?ðcˆ¿ÕŒ¤‰óÅp¿çxíztîÈ?ËÔÁÔiyAGNbll?ïÏÆ¥¾?uAP1§Ð?e—jðX?l^%?·È?k4Zl	ä?i.±'°‰?ïZ¶ø
y?˜ò›¶Kê?q΋8a×?tzëk6òh?JZùP?–=Çb*?î\PzI{?"IöÈñ6?—ž	§ö–?‰­«pòá}?œálD‹p?"ܸÑböª?ï	7&‹?–[õŸ(û?^+°
ø†Ò?np—oÛH¨?œü>ÇñA?•¯›ˆ?ïñH¶ÁâR?Véµa[o©?G˜Ž"Þ?LÙôÌ®s?Q¢K0h%?JÁĸۙ
?ïÁPƒaZ?x>
=ÏÑ?`ž½'ºÅh?e•æ÷½[¬?w_¾å*'?wI!#i¦2?ïNGæã=?'	'	æP\?†Ûì{É?yú…þkZ3?…¢Ð;Ÿ?s7óÉÿ|?ïÏ¢°w4H?r凳…?@»¥Å8d9?EˆÕ'Üá1?v3m{¢?pù'ë7 AGN3FGL J2248.6-3235@+}ÿ	_ûÀOué_ªŠƒÀ:ðôÊAØÀ;ñ9F¹?Μhv66@+渱7@"à{*n¿å´ŸzÀKÆ¿êD¼…Vìv¿ënL´cŸb¿ïýðõºÆAGNfsrq?ïÙâõê9?v¬¾´æ?LE߆+‰a?RhŸj?oÑ¥CWØÙ?u''•$ÿ¼?íÞ?_€2?ªŽå¢»ê?•vϟwðv?–«yPk‹?§`¢7e'?£s`aù÷?íÚ§Dø?–Šö‹¡? åY…‰?¥?‰‡RS»½&?¡p6ÂÔá?Œ"r¿¼Î:?ê²Í$é÷Þ?¯¦ö&÷áZ?±öf,½tÖ?¢b~NÓ?¸s0¬`¿µ?¨+ _F?ïèF˜ô5Ð?i¡vàlžÝ?E"™¶'?FT¡úñç?bTcB9G_?g,"bjÝ?ïRüólZ?½»¶Å?}ÉÇ^vÌq?yœ¼Ý2Œ?Œ[ßmÆÿo?ˆ«&ïΝ?îßEBTcZ?":(¯q~:?•+ìÎ?¬?z0†ÕL›5?ØsƒŒ:V?u¸Ó>(¡3?îÓ;7áS?Œ¸8)âÞ?À¨.æP	?|»‹¼Î0?"×ðô½"?‰CIš—Š:AGN3FGL J2250.1+3825@X²à'¤À2']ŒúÀ9(&¶ÂÀ;WD²·wÑ?Á½À´æ|@¬ƒd?þ˜¶?l§s¿å°6E®­I¿ßÁpïg'¿ÞóSãñ›¿Ö2t}xAGNbll?ï²Oºõ¬6?‡4²í±&‡?VØ*zI¹?R/¨""Ð?€'ýûs?†/lõ¹º}?îîÅÙF5w?¤Ð~"ª?~Ñ"R@?'rŽm¹'n?šs2Ë?¡éõÆ¡N?îH¶Ûó[?•½ÒQÿ£¥?•;ð÷†×?…f*™k'j? Ö™Ò•å?ŽD 0,ª?ìá#ÀhTA? Ü
¯Ž9?t…Š(òl?q¿¥Ç L¾?·¶y£TåR? Šà©"v?ïêUaŽîÎ?cS7¥e?CÒ±<å³B?= ý]æ{W?`µò†"?a´À´4(g?﶑º°ž!?'¸ú¦-Š€?d"ºNÕW?bŽÍ JÐk?z³Ø1i+?ŸfÍhwé?ïX-KÌ0?|æ›2©~?'½-nzŠ?rêZî¸UÚ?‡7Ú<S?q0Ž4­þù?ïŦV°?€TÐynÃ?f'‹ç¸?T9ÜWâÉ?š:uðè¢ü?UÐH¯ª©AGN3FGL J2250.3-4206@v"Ÿ×¡<ÀN"¢¿³ÖÀ9½Ì'ãtÀ;À4"\B÷?éž©4'‹@³-QFï~@D– "Hr?î?Þù[\¿à5û×ý,'¿âžì>Ø¿èj'–qñàAGNbcu?ïÛï±ö?j¯‰gÈ?bÆ@ãíG8?c°'ÌžÎ?aJ
wÖÈ?V_"k5?í1§½s¾i?±¼îûyG:?LX"aµ8?Ÿ%¸Wg…?®?Wãÿ‰Ý?«ñ¼~¦Ú?îŸ$Úÿ?˜«ò‡}€?'Ýóã'‡L?"Î¥W!€×?™=‹ŸÝŠÈ?"ëÓßL?漒1ñ>Ç?¸iãÍF#¹?»º
(BÐp?¨O'´¾§à?Ç0°¤œ¬?´¬9é~á?ïõ;š/í?I	>²*Ë?BªgYÔP?>]…< ‰ç?Hg}˜£?=nõl<÷?îáfÎÚÝË?œq
["?‹µ¬.M™‡?Ñ›Ú	Íé?•øPžAÙ?'ÄÏ6æDc?ïj?1vÎ?}öÍ&ÿ?€ê°'Cú?rà€‡É"U?"…ƒ¯²*?u‹í*¬¾?ìθ ×Ñ?¢)˱gî0?§îèþÍ-?ãtM¨4?«%Œñ.oÄ?žUWÄcÑôAGN3FGL J2250.7-2806@7½f@¦¹=ÀO§¶€Z-sÀ7ÇtZÏYÀ;[^Ëgr?ï½icà"î@
Ő¡@k(_ššK¿àT¢pN¿¿âûØZœë¿ã õyÐa¾¿å¤ÓFíÿAGNbcu?ïüûz+¸?5㚣,c?
Eøkظ?¥ pY†m?9풄T0?3×۞¡Á0?ï XÀ`'Í?†FAs`÷?aÉeÆ·ë?g¼EÄo?ƒwvj¨²í?'ý™
Œý¨?îÊ¿¯#o?'*í2€­P?ˆüH{[?{£r=»ž?š)øáxŒv?Œžƒ%s]ï?ï±f#fº?½Û•*Ê?0"؝¬³?AÕӘµw?ƒ%''Iä?Žû¯5M?ïþÑãÚR?"Kß+1E?MT˜Òú?ž³7Y‡?&¬7ú»V?;‡¢ÎaÚ?ïàäÍ°³£?lhÿªþé?Oq¥G¡(à?Qm'_eLR?g>É&!?eݏG2ö?ïmJv?'ô#¤&î?{"M3™ÈY?ptç$;DŒ?‡.T+oRE?\º'è?ïîæ·³ê?`ß1âþÎ?#EòS擭?#¾Þ€‰^?_Ë^o-?_]ŠI"äAGN3FGL J2251.5-4928@uJ^`=WyÀLú`à¨.À9³C½Äò
À;¶V¼¥7]?îyù$]q9@©;"@?ÿx®àR»¿âzï(‹¿ÜSLÙ!š¿Ô§RR:èè¿ä%ržê!®AGNbcu?ïËÛcq+?r$
lJd&?bC¹ó?]
4?]?pðqÊw!ê?j»̓A?î¢ÜÖÛ•? ß)cÚ"©?ˆgo-'é?‹ÏER8"Ä?Ÿ\±m#í?™˜ÈÌ'¯s?î
´*7Œ?œâĚt?™mðІ?Š|H?¢ž3#œPÿ?"÷îkT?ë™Æ¦3?¨`ã.]íc? 6"Ãtg?˜8(‡Õï-?»™0?¤gï1ˆ%?ïçvBÑ?aû9-[uw?PæžÊÐÝ?O¸¦‡Ô'«?`n½á2?Y µ{¦*S?Üoà–?…«€êX{?tXÅøŸõ?qe¥7eԒ?"È܎re?éüÍu³?ï4ØËnäö?†Yv«èW–?ˆæ7;‡hà?|&ylú"}?‰ã•áà!—?už!S
ãº?îIþ÷Aj"?ÃI®_\?›¸üM?ƒ_.!p$?›CG?…}‹}xAGN3FGL J2251.9+4031@Xè#¿ø¨ôÀ0àé_ªŠƒÀ9:$)ªô5À;‡Æßî¿ÓH:õR¸@Iá">éu@þh`f¿äÊD;œ<¿äW§¢¬ùÚ¿ÙéO¹?–¿éí'u¡ÓáAGNbll?ï–@1?à?ƒúEã-q0?}qF­¦#e?~´œ¶ûÆ?w‡QÇ0H?rŒÁ› —Ö?îƒGˆ)ښ?©oàG.æé?Š'`Ühë?ŠýORvæ?¡+¡» +?¦dŸb—‹?í6ýÎކ?¤ojo™ó?¨áÏn`Ýp?ýzà3ˆ?£®S¦Juþ?'Ý$/u"?횝wõ"ý?›C\pû2?}¶Åü²nV?u"ûKi ²?±O§ÞÛáö?š99øî?™?ïßA}'–µ?fm¥äÿ?a[ߥȡ!?_g—cÀa?^ÅFr£g?Wïô¢WB?ïuӔš´Õ?'€Ò}?sš,ì?q¦6%ô?ˆ¾ßKx¦?)4ÜÊ~?ïêŽÔš?Œ¥n],‹6?4—(©?‡'z~fÜZ?ˆ3Wˆ;w?tðkÙ}?ïelÜ!S?{æé<qÛÈ?eÂMrǙA?W«£åÕ?šÅi†J?zxíåfÅ´AGN3FGL J2254.0+1608@U‡Å_ñ_ÀC_ÏspÀ4ƒJïèZÈÀ9ñ´Ï€t@7PÜfs@&LÉn¯?ÿ¢F…‰A¿áÀìªkV™¿ædˆ­ZŽ
¿æ˽ eí¿ë§òX*A%AGNFSRQ?è®;Qº²Ä?É`Ë- °¶?µ£ì‰Ï£Ì?ÁPûä#ö?Âuu	J	?ÃÅbÏq܀?ïp,'?¬h«O¤ƒ?o!§Û&Ýß?•ÍMä	`?Œ,qvZ'W?©ÐZ
ýž?ÕÏô<°èô?·µ¥¤÷›?Òõ!–8ø*?¹¡ŽHÑ?×:ê,>#?¿Ž››žÎÚ?ïýK´x1?Rd—pªÑ>»çä¥d4î>ÞâÊQ)Hã?5†r5n¨?RdÊ¥˜9ú?å#Ôi	•?Ð߂DpûÉ?½®FFWʏ?Æ©ö*‹'?̜‹/ôd?ÍGzNOÄ?ïËò'ûÑ?›,–y
8÷?cBK®o	?Žú•~–?p'_gÏ?ˆœ"Sõ?Ù#	¦-7?¶Ê»îÎt?ÒÐg/E?µ[è™.?Ô?£ƒþ?»¬X›?ïÿn…CÌ3?63ºÖê>ÂjÑA#È¢>ï(þ*å?œ_ƌï?6(ɇ ÃMIXED3FGL J2254.0+1403@U'‹ŸÛÒúÀCõrØœÀ:0<îÀ;aC§õ|ï¿àõÖã?ïž@Uö÷Îÿ@ì‹àžeÜ¿æ4»ÚåÄ¿èÖN+î+¨¿áô%öø¬¿É#ò)ŽÖAGNbll?ïõ)©OM?R}R…żŒ?3æü"Ó?:ÓcrsÃz?Qî`Ý]?OKœ»¼?âãÔ??…ŽïPÙ?d•ódû?g}1킋Ë?†R¢ÌÖê? eƒ§ü?î¹YÚß+–?"‰X3Ü?‰D»ì‹Ì*?t¼JzÍӔ?œ2f¨­="?‡Ùcà?ï>Ûc?Ýx183?$ÇÆ«~IX?,1¤ÊȎ@?Ÿ.®}Òã?p–AÕ L?ïû®±¦"6?>Å«ÿ(Bµ?%µ¾Œ·?*×»"˜#?8hØ©}?7òÒ
Kõ?ïÛ+4ê ü?jOaÀÐòL?QJÔؾ]?P-bꏠÄ?l/`~d›Ë?eµ™îß?ïˆá'D4?r'{â'¶?vËoqÖEÂ?d·*:ý?'aþn Â2?j5V6¸	Ü?ïÇfÔÓßï?i
-|œª?Ì×àŒé•?
{¹" vd?{ùb&š¯R?hðQ–à~žAGN3FGL J2255.1+2411@Væ æÀ?ƒ:€.Ž‰À9_h-æÃÀ;€·Á¢Í¿Ób:h—Õ0@Œ—[Pޕ@'ž‡t©¿Þ€ÔñßUæ¿ÏÁô—1›¿æ:'Dˆ¿Ú™ó¿ˆt6AGNbll?ïø'ìHŠ€?FeÖ§e$W?&ƒ((›çô?#¶ü¥ÜÞ?H"—5çL?DŽV>ôH‰?ïŠÿ‡‹}?‰(tŽ(i"?d3‹ni?e ЂStÏ?ˆÑ_;?†kÁLćb?î¼…]™Ü?',KqU±?"Ø*O?‡I


B?•~¹|4šA?…›g4 k?ïqÿ''Ó?…HÍ@"'¤?E#A»ÆŸ?Hð³a?'õ«anå?…6jœÂH?ïûc¤48?f¾ß€ƒõû?"ÂþÖ0ÁÐ?H?"¨íÁ?;†$5ši?`À—
yOÕ?ïÖoŽêOP?q8aFÊg?SÊ¿0?Qp*F¼Þ0?o«e˖(ç?lÄüLf?ïaòYµd7?†¹^‡ªÙ?†Ø(™¨èT?"H±Yê?€«@ô.–?v¥ÆÐ=Øn?ïáäT¹üÍ?a¢¡¥^û?%[	Ê¢?2ªpA?lÅòŽåwõ?al‡°íüAGN3FGL J2256.7-1022@M›Ö_ó…žÀMCÀI0ËÀ9˜OYÚféÀ;à,/2ór?ü
߬ùH@¸åå!­?ùrLK:\?íN'˜Œ¿×lôS¾1î¿æ&äv?U¿íšpÙÃPSRPSR?|=X g?}ٓk?†®?ïV70\­ð?—\¹>z?ŒS°5¥Cë?"*Ç/?¢§ïýç<‰?¸—yªwª?éï>ÿ¥?È(°oÁPd?ÙæNdM?¼Yç@Û+?·÷6ŸŠ†?¤pÿ"ëÒ?è{S"º?±g½\R?Âù™½'?«"ñ`½Ë?¢ÁyŒ§Ñ?˜GúqtG?ì·Îwh¨?®I"߃&É?±8.ç~fÔ?§hQx¾¹?}Y3pN¬?•Û?Ùn?ïmŒ¡Rd?¡éuހ2Ó?…ó	£+?›0cWå°y?®± ÃËņ?¼{
ß³ü"?éSÐùŒ0?ȳó%Ä­?ÃséB	¡?¾v'õ:ª?Ë8"ÍÛH?±ùêê?åžèï©Vâ?³.ô"0?¼ÖG['^?¥L1N/"?¿Z#!˜+0?¦è'®¡q2?ê3™áy=j?­v²+9SY?®£"? <ÌgmPSR3FGL J2256.7-2011@DÈL€SÀOt?Àà0À9HÄIpŒZÀ;—¢çöô¿¿âíÐ.q~@
/óf¿|­@½}ÿµ,r¿Ý}Ì¢8,J¿ã[úk…¿ßp÷TñÛ
¿ä¹±~AGNbll?îQØ)Í-ñ?£v]™À?rÙÙÚå.ç?qœán
ÇÊ?¨‡B)ö<–?¢Õï€ûS?îŖ—Ü€?¯Å†"Úhî?…¬3n$Gs?™R
þzˆ¡?œwIî<‡?¥lBØɃ?ìí©±ó5J? ²,œòè¶? -"c·?Š¶ÿžß"?°'¯~ S?š"LáV²ï?ê­|yg
ð?±à°7#?Æڞñ?I}Ø_?Ä-¬ãq?±§=
€î?ï¦j!z?'>€#{‡?XVѹÁ»J?V‹ÁøZ?ƒn<Db?€¸ŽõüCü?ï®wh±:?ŽÇ]žüÔ?dÐr)+]'?mž>»µ?~\q:ž?‰DLD®)?îêC(&m[?‡&,Á D?ŒqF?{¦¬1`È?"³âžC…?€} a©N?îƒCEÇVä?"_»>"l1?dÚ½ó5'F?Y>+•Í4»?¦~ÈJƞ?"*µ)BAGN3FGL J2258.0-2759@8ZÝßCÇÖÀP:B×P´À7¾Éãä@‡À;=ĵ§Z@'ûE[(ñ@Þ%™Â‰R@øӞM2Ž¿à¾o'Þ9\¿æ—ò_®fZ¿ç:c‡Jë¿íD¿ÇžPAGNfsrq?ïŒéz'}?ˆÐöŽMq^?‰BEÏáâÛ?ˆmEðÓ{ã?\ÜÃnŽ?Sc+*žŒº?ïŠ5[]Á?;ÇÕÜ?hQi&Ñ¥K?nH¬[YN?‡^_ÞlDg?‡MJl§÷j?ì˜E›0?©(Æ¡#K–?´âúó@Ü?¤¿°,¹P?™kd=qn?"²ÙeõBÜ?ï‰X*°Ð?'Yz¾¹Ãî?`–Á¸õ'?qr'ËD"?‰"Dۗ¹ò?d²öќÚ?ÿ>Ræ?Ò¥ÑK¼¶?…õG_òo?;‰˜ð|T?]ÉàAA?VÑ<Þ®§Ã?ïÎ.ˆBs?uËä%I1Ã?Zbá_ú')?ZúpòÏ÷?rW°E£']?q§ìQ÷?ë"0¦]n½?®ð€+ð"ô?¼yµýÂ&ð?«ƒãT»U?›³?Z?•ºu!ä-?ïå¦@­*?qŸO›ó?So9=u@É?T±"éÚÅK?`¢"ºúN?nòWq3ÂAGN3FGL J2258.1-8248@s04ÿ†]}À@³€ KÏâÀ9‹pd*À;vx†?Ò±ó¸Ê@ÏZs@ŒóŸŸm¿£q³üª¿áÙþú±7¿à&Ì¢Qñ\¿èUj3`»¾AGNbcu?ïØ£À9 ?gº-o›4¢?cJþ\6½?`Ì—Êå?dAcÃ?X¶AQg?îžÎ‡b	Š?¤"N؁ì?…TŠÍ¢*z?‰©Hû? ½ôÓ@¿?¡­ÚçiF›?î_k(©(?"5yäâ?—OdßV%÷?‰p¤'Ö´'?œ¾­Âsí?‡ŸŠ.ø?ë}¯?¢¤S:ri??–Å48R-?ƒÄÂAÏr_?ÀË@ýîz>?¡äÕé<UW?ïôÆ?êô?K»Ë2K¿?D"÷FÎì?B‡Þ½–Õ?HSÀ_¨W?<CŸP=f?ï"ðo
Ç&?‹Çÿ˜V?q²iý¨?'?q÷Öێp?…ê¯0»¦ã?‰ê),ˆÅ?ïhA¯¾?{¹¿…ºµ?'Ãc±œ?sÝvš?ƒ,0'MP?lÕGµO@?îtçÑ
<?†›°À¿³?‡žEÆuÕ ?iìý…ƒ?¢Éñ{,ñü?…3ŸV×YAGN3FGL J2258.3-5526@t®÷_²íþÀK'¡ ÏÀ:zi
à"SÀ<ë7@?ÑòG" S@Ò3>íÂ@|®¸'¿æŒà/¿ç[î¤ý"°¿éÝ=K˜?»°fQvHAGNbll?ï¦cC=¹Á?‹
f²ÒÕÄ?ZïEÊCî]?^n<h
?ƒ	Fryç?Š/9³½Í¥?ï'è4?"›5;{J1?jdt°>iM?{IœÂ+?ˆ¬Ý<]]¼?Ž@®ø¦ò?î-¡ZO¤?"Ù-òñ=‰?•ìT±ÅûÆ?" h¿T?¢8ˎäRÞ?ŒŽÝº"?ïI¬cû?"{§ÆLð?U鴌«žÑ?dÆ£žCb+?•kâñ	>®?'å½s8gî?ïåý÷Me?lh,^·¬8?>U=íÓ?=Ù±b?f7a£Œ?kXã-¥ÂT?ï×4'-êt?qªÀ–/B=?TÜ
ÞÃ÷?WאšIqS?n]g®ûË?iþÚ©jÛ3?ïAào¤þ?'W9¦Ø…?…æCi¬Ùø?yµZìêâR?‰¡¹sŠ®s?vº-oó*¡?ïé¦8}8Õ?eÚȧeíj?8©OµR¡æ?BëRcÅ
W?cDl£ž?cWn)#AGN3FGL J2300.3+3136@X5 "ÚÀ9
¿v¢õÀ9Eˍ1¬JÀ;df\Ukl?òˆ–i¹W$@¯¼EÀÿ?ý™ž>ÄáÇ¿ãŸM›lC¿Ì-H"÷Ò¿Õ-	²u!"¿ã~bª€WåAGNbll?b‡M?
'­E?j½Z"ó?fe`S"*3?€£Ð»Uf?{¥û,Q±¿?îL2¢XsÎ?¨òð0?þâ£Â  ?Š$‹½ì?£=2d?¥n¯3vg?íyn⎆?£,["‰\Î?£î8_öhZ?–'}p™?¤zـˆ}G?™3­k-‹?ë²ÇGÛ??¨"
Df1C?¢®L¢þ™º?š•©cÕ×?¹«u‹³­?£¯øø*#?ïÝûéoð©?ièÛG <l?]ÐD•¢k?[ü\'›?côr™'Á?_oúj?ïN|»E—?–Å+;臘?|oÚ¢:¿?vÕ]"V ã?Ž(ãÚø?'˜,Ÿ)Ø??ïÇ1_üó?ËCGÃÝ?'hNT+?‹¡ßâb+?ˆ=–õ‹™?}¯ŸªQ»?î0Ú¾R?j•šèkg?Ÿ	"ww¢ý?ƒF;'8H/?0Q('¸?…ÍÑû">AGN3FGL J2301.2+5853@[Fú>¯h¿ï'DŸÀ9Á¾òïvEÀ;:9%»{l?ò³ç®O‰*@åÆî¼a?ø7¥þ׶á¿Öæê…Dwÿ?ïþzÄÂ<P¿ØŸa´ü¿×Á›@bÇOTHERsnr?érîQ#U'?Û¬!K?²W£þã=?µ,#¡'-â?Áu5rcÜ?¼Å©ñ?ԉÔcÖ$?ÔR]Wó¡?ÀY?P;Æ?»˜Ö2«Ú?áºƃv[?Ó_"Ÿ•Ã?輪ãg?±"۝n<(?ºüC—À?¤ex¡ùU?¿§­Oü9?¨…ûԍ–?ç`3Ä ¤?»•Æü(Z?ÈÄy6w¶E?¹›ñkEPö?³uoq©šÖ?¯Ð™ð]sï?ë·=ðÚ?½ô8·²­?«¥&_x&&?³ÒßÔo.?´tŠà¾þ?´;¦zòr?á¤ECè?Õ@º¡7Xî?¶Ä›Sl´?²?em›x'?×ÎO?¢?ҏÄI¬­"?ìqữ?¢£*úÅý?®e§Ìþ™û?š\<Ƨ;?ª‰:å?—«_E´	õ?ëI
…x?§T\*{¾7?½¶qÁÞ?¤­™Ê¥?¡MêЋ Å?"jÁG'ÇMIXED3FGL J2302.7+4443@YÙN wmÀ+ù¿è,À7ý£ª"" À;L(T²ß¼@-ù압@h´Is<?ú'òg»ü¿©ÿP¶.ƒT¿×ÿ'¶•B¿âs~õõ¿ìß²ÔPSRPSR?n¸µô…+Û?t§{-?ïтîÔ«á?{Üïí&Ì*?_ˆ¶xœ¦Ä?c"s_?y[:•}'C?ª)ão¤É;?í…üÑÙ7?¶ÙµHKÉ,?²:eÏL4à?²ÓX29?˜N}W‹Û?"qú+EL?ì͞씾>?£Kê»Õk?³"ºL]? V3m‰©?†(ã¯6?€Zˆ9…iÚ?îsQY˹?š17Ì+á?£@±œ«Øó?—™AªÑB?`م?ãüY?r¤fmo‰™?ïå&¶Uō?v(lÕq.<?Sÿ‰)ã<÷?U®™ ½?x?à…†P2?ƒ´êÔóî?íKû"˻?³çKÍ4°õ?´#âö>g?³e–E.æÑ?£ð¸}X?—ÊnXºö?졏†4%æ?¥`jAA?°û'ÅØ ?ŸLÓ	«9$?–¢Kç+•'?'X:ó~¹Û?îù^ju?'¹é¢äÀ?™^ˆD´DS?Š#åò PSR3FGL J2304.6+3704@Y^"ñÀ5"ÿÖåUÀ9q¬'$ZÀ;iQÝBeÖ?Ýí¾jŁæ@¤Ô…'ò?ýÀŸ¿äm½å ¥Ÿ¿çÇ"5¿ÌèZ²Ì¿²<´fN"ŒAGNbll?ï÷A2­ÚÍ?HY˜«ê d?%Ä•8Q!?8Z©:_é=?MŠ/™'§?CÞÀ¹y«Á?ïy
`EË?Ž«¹¬´~w?p]Ïa$?}9~Q@ƹ?‰®¹kþ¸?†Ü4£êŽ%?ï4š.?'®7.Â?}|":g"ô?n1ՈÐ?'·8ˆ?~Å\ÁøÚ?ïªÒsw?'Jê)ÁÿÆ?;'ˆ‡éÖ?H½Ã¦Á
h?œÄ| €â?'7G\8y¿?ïôúPÇ n?Œ×çφâ?LkàÁºqP?'¡äOû??U·+'ŽS?1ûU"8?ïÏ€·±™?qyy©Î?Yª.PñI?UeF9¢ôn?r
´)þ:?kÒA>è~?隸>RÿŠ?p
ý›j?q.ª=¥ÚÊ?gáÂñ¸YÅ?{u6ˆ\@W?d>k‡wØ?ïÍf¶Ôy%?kóžÝK+?<>¢Á1Þè?;qò—õ?wˆºJ}uv?j¿ÒN}<AGN3FGL J2305.3-4219@uîCÀ~à±ÀOÎ*ŸæºµÀ:ßNG‹¯ÌÀ<]û]Ùпê/wAÞzR@
¹µ.Ëo€@b¿g£¿í ›:¥å¥¿ /-¥ l¿åoº 9¿Ú]2p?®AGNbcu?ïàç_äÛÑ?j¬r€1ä?Q}Ç}ðØ-?`‰"ƒóø?fY¼%2%?aµÜbò^œ?+ëÚô?‰V¾Pþ¸<?c§ö
>Ö?e™4 åÅ?‡*7y"‡"?†Ï5˜úI?îh/`¸?ž4š!º÷?"È"?()?'+‡G{wl?Ÿ1€¤¬Òn?†5€Bð~?ïžÁˀ¶8?~÷Žë3ué?Iƒ/×mÜã?Iîb²4Þ?†·ZÓ¾Å?~fي?ïóš8rY±?Qd(9–?2-<:L8ß?0¼5¹j?T@@"ÊÚ?OgŠ[¸¶?ïÞÒ¤¹C"?k^r~."?NÊ¢'•%Z?P$×CÖëö?iz²niσ?e®(Õà¿l?ïM¹øší?zäßÀ%é®?"¾¼€Þ¾?t>×"øž?‡ÒÅN)?jÝÎV"?ïî¾IÚÈ?T¥©ëFðŠ?%3!Û<G?C½iiB?_Ý»1Û?Tª­àAGN3FGL J2307.4-1208@Mµ?Àà0ÀN±v_Ø­¬À:‡kþUÛÕÀ;Ç%l¡¿Üø'y'Å@q!Ôæ÷›?üXFÀ®±Y?è@wO€¿åFðqdÆ¿èC,f ¬"?áQoß6öAGNbll?ï õT†ô?…;¤.¼å?O,'ï
×z?TÝT?…Ïք–5?"Ä,Ö|íÊ?ï–*aR€?X– ·J?gGí
aÍÝ?~>üŒÒd¨?"¬º1	zb?†œ½[,ÛÝ?íæ)6§~?›¡¯É£ü?Ú'SCø?ìóc'?©T­£´?"ÚIª«Ö?î–ÿðT€$?¥ÀÎJ}#?A'ô"a*?V#ï@èš?¦I¹'@›-?¥‹?ã"^?ïäc÷÷?i¥ÈÂÍ'º?>•ÆŒHEà?BŸØÒ3Ý?gÉOk…?g«>7–?Ø?ïÙÎ$]#ê?"ýøÚ?þ¨?UFë8•l?v%¶rõþ?kŽÒȼ«B?v1<D;Y?îÜd,ØÙ©?Œ¡}Èúþ?œß'º?'mÛ'ëðÁ?"ã݊Š2?ƒ¨"žäd?ïÌ`Õ(?vðçV	z¿?QvN¢¯?(†¯,ʓ:?y~O¸cW?vĤ¦½?xAGN3FGL J2307.7+1449@V5X`fÀDŠæü9¢À9ñÝ'ŽÀ;gÝX5K;?Ï$¢v·íB@lÏ$ÀԜ@èj#ç;¿â}ˆŠ¿â˜@URb¿ä¾Æ³>lˆ¿Û³ÝF[rÜAGNbll?ﯰ)S
"?|[ºÁx?oáÌÓ¡?noçÄtäƒ?x£âÞµ8?s[n²°ì?ï·ùùM+?Ÿ^ÍV9¼r?v%èÁ­C?'I´Ï_	4?—†ÁýEN?›]Þ¹{­?ìîMåÞc?¡ZȆ=²˜?¦'
üpD?•á²¯a¤W?ª™£ñ¼d?•
'èðûÈ?ëoýѧ}?¦lñ\-M?Š$Al «ö?…C8Wíú?ÀÄ¡… f?¥ÙëP<û«?ï興¶X¨?c9cX?T"Ä2™å*?U–(G09?ZÌ*šn9ô?V(L<&}?ï·ÓÖÆ?'ÆgŸ×t?b(źÄ>?eY@"ƒÝK?{c³n‡?—),j0f?îè9:fá¿?Ž"7†‡?'2â-ñ¥«?…³.{ë?Åö~Rê~?zr:À¤?îÂý–ZÀ?‡ŠÍªÁÕ?v%…G=†g?do÷Zÿ"à?¡uóÚÕ:?†6¨™ÍØAGN3FGL J2309.6-3633@Cï@j(hÀP ½_ÜßjÀ9øÀysžÀ;­›÷Aë]¿ñsCÄzï@]¸šºx?ý«¢¥é¿é«FuÔG¿âÚ2ÚKæ¿Éð'ék¿âD.ŒÊ*AGNbcu?ïó¤FÞâ?z5?‰6?¿Ì4†'3?`:@Ô@r?WÚÄ$9H?zŠÝ²Vã"?ï¢Ï=?{–?ˆL6ªÛ5?c‹Úo=?sGåÛ³7Ú?'ikwè?Üa閿?ï4j½…~|?'
‹ï>ì?€n `Ì3?h|žb1rœ?';œü4k?}õåÌ7#?ïaÄvùé?ˆà'›ÆÄ?YýԚ›?!½±ê@ˆ:?"¯#?ò ?ˆÑ@=̃?ïñþxҊã?"@ÄMµ?ë	ÂÙqÍ?e?ö?ZÄ]'.:?"AÄÏ??ïßßr°p?j_î؆X?P&º#u<?QEî"ê/?h
0r0ú?cµ6¤°?ï£YF ÖØ?p–#E9ýö?rJ–U².$?_Ū1×êh?|ÆL#õÌ?jè8Û`/ã?ïÝ¢Ý\‰e?`@H]§|?

~>öü®?ÕÖô?pú|sÉr?` »ÌFWAGN3FGL J2311.0+3425@YPaAcxÀ8_€™"À7‹áP°À;&ûL<µ?ûz9.Êó@3¼]éÀ#@㶿á™üL[7¿åWʯï¤ò¿åY‡lÀV¿ëÌkŸÐRAGNFSRQ?ŸhT?ˆ³Poœ)ž?"mÈ-tc?ˆ0r¯7-?]!""¾¸?U8̟ad?ï‰0b?݈?™k"¥M}?oaÃnF0?~>8‰"/?…Ûv'_kÿ?ƒê‰!WŽ?ìؾҰˆì?§A'ÑÁV·?³%óèA2Õ?¤)+¤Fç]?˜PV
¡å0?'w,_ĵ?ïï/w*Ț?k‡ÒàÊ´?%
3m÷W?Köò~A?^ÿkÁSKÉ?jr-œ«ÔÓ?ïÒ×î"ñå?q-AaUM?ryŽG:+?oëJº,ú?Piéôìù­?J³Ö½"?ïÖïÌà,?pfÀà?VÇsòÃú?TàÆ?œ"?m¬yùžÅ†?iĄ'k?í­‹øW{M?¡#<+eš ?«l{Y`Æ?œîcJ}&Ç?"uŠDØ?sA'Dp?ïýa{ß¹'?E¬VÂÿÎh?²ƒaVvX?Ý!.úê?1}з$[_?E9P'ÄZ9AGN3FGL J2311.0+0204@SÔúÿåþÍÀJ
@TƒæÀ9ÜàáVǍÀ;Æ)}§ËŒ¿ô
ý\aªÀ@d¿o—ª@+b€R˪¿Àâô:"¾}¿æÕÝCßË$¿æ˜	Œú¿Ï¯7¼AGNbll?ïõ½ö‰ùW?R=kt.p?3ÓWÅ\r|?7­±WóÞ?Oyû-Í?N9›®õ'(?ï|yñ'/ñ? /iV7…?eÉ*É´ÁÍ?wðë
uK–?‹o8ô‰.? Þ헺Ë?îÞÀþJ?Œi/Yäì·?·'ÐÒ¶‰?€œ
˜œ?•Lk
-q?ƒ/y֊Û?ïµO _Ø?Üït4ŒÒ?¼p!•?Œ&ɋ E?'"u/'nü?ÕÀφ#?ïùW›Xœµ?cöªÕJ܇?.FëWº¼Î?II À.ˆU?C×Pß/?\j㠑A?ïÝ+·"ÕŠ?r%tٛ½5?PQ*dÁI6?R‡É×?j«²øǛÅ?n"96â¨?ï€qYUÿ?{ÏÒ7'c?~"GYÜx?pBµ‰@†?€Ò…÷bæí?tWËϑð"?ïó‰V¢Æ`?S-Û@¿>ãG^â/Ë>áÛ²ã`6Û?XÆÄÓÅ,?S ±B±/AGN3FGL J2312.9-6923@s¯£¿ø¨ôÀF®v?ø="À:Ë-œ}ZÀ<	،°?ã›U"Iƒà@
^,±
ÿ?üÝK?nå¿ïÿù?Ð??ïþÔè‹Uo¿°œ§W¿ä8tƒ4¨SAGNbcu?ïäl0w9?i+6‰??"Z_!ñ"?=Ûc)¼?gü(Vùy?gÓ|žŸˆ?ìÈ"Éþ?µ R?¡N±æq­?¢wJÓ¾?± ¦E8?¬-°Ât?îaƈÝV)?"XÝwûöA?Œæ‰Á4?zÃôΫï'?¢ÀÑr?áW'Ϧç?íÖXؚq—?©u×Ûd8f?§#X"vÙ?¦ŒØ¨é'?–î4»{i?—]/AGYA?ïðޜØé;?`3HjqŸÀ?-
–´?/'Ð<bñ?Z'¢ÓØÆ\?]ç0ߜŒV?ß\ò?œ{H1g ?‰Y·+zØ
?A¬Ë†™?'³nVõ°?Žú˜†ô?ï=e6n.º?…š[o?}´:³pâl?i¸Í<Ç?æJ†½È?ƒÜ…ÀáiŒ?ï7Ã-fÀ~?‰Šû•8ì?"º¨"—†?…ômý=ë¹?t~˜×'Ò?m£ð¢üWAGN3FGL J2314.0+1443@V¡ùŸÿhÀD÷"ßÎ1QÀ9Ž—rwì¡À;f"Ú<ø¿ðÃðBÛ@Ýá"êµì?ü \†ã‰¿'îâ:6 '¿Ôa÷8R¤¿ßï§yu¿¥Šòóä$AGNbll?ïÎ3rPÝò?yÁxÀ7?S"}–$åS?Sb%Me8<?t'"
³?x:ªñé»h?ïŒnZчÈ?Šíxæ\&?gJ҇±ð•?{þ0–!ŸJ?‡´¬qAõ?'c¼­bÖ¼?K•L$?Žäô§U?'…x×*"k?'ò­ÀÙ?™‰=»SQ?ƒ]JLl!·?îãL¨5z?"y½¡¸1?* !«ã?é?1&ø—è÷?¡´ÖӃ?"pÇ(Îi?ïìÏÐH"~?j$bº§1»?D–z˟Î?d_Ž
8Jò?\"Rm'¥?_ÌCu'±s?ïÚT÷Ëu?l¹jjM?R8´Øále?Q?ǃY‰?lŽ­°¼pÀ?f>hL¹?ïmp/à9Þ?xy;¬.Á¼?ã¶)d€È?rò[@XŽ?'À=×UÙ¨?iw!‰7'À?ï»J&ûӇ?nÚn©‰"V?
qæÀDÇÔ?•³¤?e$§ì?nΡ‡Pv"AGN3FGL J2315.7-5018@tê ßÞøHÀNAY@
6IÀ9»˜"à5À;Êd¨ E?å1®v©S@
ÀXr‡ÜÙ@†@.l?ï+šeÏñ"¿ÞtXÔ¤ÔÙ¿åmÊ"Dñ¿ëÒºŠUAGNbll?äÃKºq3'?ÈÀZñ'?Ò*(¡Î‹-?Æ7š¥L"?±<ÿ£"l?¬Ÿqï¸]u?ãB¤ÏÇ?Ìã:Ø/w?Ìó'	YE?Åt~ËÄf?Ædx{Í?¾?M!4ÇÍ?èiK1ñ?¬aIA?Äsm܍›E?§›®pñ?³ÎÊÀz{i?šß¾N×>ñ?ÚÒJÚ2ª¼?ÀÕ±u¶îó?ׁý¤9?ÂH#ŸX?Ë]_Ey š?¸VA®Š½??éó~«'ѐ?üó®ìo³?ÂᶚA›g?Á¦P·(?¥A:߄Gh?¢ç³jš ?éCÄ6¿ôf?ÂBˆ¨R?À-Ú§4?¼Õ3'mo?µ†¿.Ki?¬/T"kô?ëƺäžÊ?¥ïÉÏ\î?¹Qc3¦×?£6Ü» `? ñ\°–G?ŽÏÒºÙ?èÝ
¤–T?°ž'¼È¡.?À™IÆ%Fi?§Ç@LÊ~¬?·åOrœ?§ð³üC]AGN3FGL J2316.8-5209@t¼]ÿÅGÀM«t`$-À:£\ŸTÀ;ޏ±¹K¿è i6ÐK²@jîªB3V?ûÂ@&¿èó(!öñ¿å
m*È"¿Æ<C_½r¿Ö§kŸ‹KAGNbcu?ïóø:þr?UæhôÛ?•»Ã'Óâ?»ñQ6Â?Xij³'2•?U›$ÔÌö?ïè
Eú?"]Kr2º?`Å&ø«º'?bÜæd"Of?"T²ßcÆÛ?rÓëÒ±ö?î³Üp%Nf?ˆçKÞb¼Ý?…%‡`øa}?l¿;ƒ}'A?žñ®Cúʚ?†B=—Y0E?ï@­]Ί?‹ô˜óËL?"k‰X)Û?)]'/]u¨?—Ň}.–?‹äã=(^×?ïùIìÖ
?B|6ùp?Ã*Ï$E~?ÈbC!?Hce÷°~´?AÒkw?ïß'gî?l|œlŠ}T?Oî.¡ƒ¥{?Q‡mbP"?hùlôè"R?fGD¥ßí£?ïmÉBîUø?uÄa|pa?y6¾¼‹g?cãkÐ(»ý?‡òOì'2?pJ.*jv¾?ïÚ/š]Ÿÿ?b'ãFÌæ?…uDJä?z4°Éü?rr=Æ?biâ7¾@lAGN3FGL J2317.3-4534@ua›«–òÀOà§`+¹ÂÀ9kÝ3L]§À;²ýî­È¿Ê$Û
ŸÀ@â%¯çä«@}1ÿò¿å"¸#G'Ë¿ä5wãˆÈ]¿×iØM€Þ¯¿åD;8?SAGNbcu?ïâ"T=ÄÝ?r·²oçŒ?/lHS4?0|´­÷¼?kæçïn·?rT1Ã
?ïtÌË	?‹ƒ*!Á»?l.¼VÐ
?o'Çõgj±?‹ÁN'§Ñ?‡)ªœ–ç?ï
ä«LÌ?ŠnÞû"?'tUЉ H?që©?¬£Å?•	?¬®ÃN?…=˜{‡@ï?î£ÆG'Rè?–T¼Z•¡?\†ÐÅþòý?ZÑO?¤ßdÿÞòê?•ø?Åà?ï÷¾I
æ?QÊà…tr?%0_"$ýM?"Œ¸Ãu?P?K¹§m¾u?P¹tÙnÞ?ïÒ'3du9?r\,?êÌË?VõŽ^;mi?U³JþR—,?q/¡˜à?m¢ã9^½?ï§èŠÔ–?q&ž°EáÃ?q…BÕÖ¡c?d{¸Ýª‰7?z†w©àÞ¯?eï.¯S?ï¹³J‰€?q¤KS,y8?Gœ}1£Æ!?8päÃe,?€AËVŸÞ?q31ªåUAGN3FGL J2318.6+1912@W£?ãDÞÀC?N™À9ÍS¿šµÀ;´¢Þ¼¹Y?à}Ç2÷v@	(ô@P@íÊà
œK¿èǚ´Tc¿èMÎɍc¿èúœQÀù¿ïþŸûˆwAGNbcu?ï­X}?¦ƒ'Dh?xÐF{"ÙÉ?xû*ã߈?p 0WB?iÌün
T¯?ëäÂpíÞ?³"¼TÎq9?¦š|4ÝA	?£®«Ãuˆ?µŒ®]ºµ?¬øï¶î.?í9§<Í«?›Î75ý?§¥"´"?''Y"*Ç?¤åézî¸Ï?8`+ªL?è9ã?nÅ?°åëÀx˜¨?¾¢Ê½}?§x¤ä¿?Àm³r†c?©!AjÄÊ?ïÔGNM?qV#áM?kd$ò©ÿ?hºù®‰Ã?`T6d	"?]3ºYe˜?îe_Io=? p l•¬/?"X!ž+?Æë'º`?ŸòuJQT?—ºDÆÜ<?hPp?‡Ä³C{å0?™Fþшœ'?@þÝ÷µ?Ž'hf©~Õ?v$Þ)îb?í±¸A7®?"0Î`I?¥&ÃÀQ?ˆO`Àì?Ÿ{w´[U«?‹`~&kÎAGN3FGL J2319.2-4207@uÆ# ƒ˜¦ÀP|Ù ,Æ2À:7_èžÀ;âØ+¥ 8¿çG²,s¸@g0¨êD'@¾àP]¿Ó&(;f3¿æ,u
Ü¿ß|c0"ŠÇ¿Õ?\hØþ×AGNbll?ïöäá¯?H³b&®ãm?!ÕÐe€³?%|†ü?Oú8Sc?FâÃnlš!?ï ùhrki?ˆÏd7Õ2?aWÜFz«G?g—1è‹ìF?ƒk®×Ñ?"r~XŽ¢?ï!	ºéË?…éu:nÚ·?†È"°‹Œ?sz*KT¨~?""é}ÿØ?€5vbÏ?ï?ª»G?Š+£s—dQ?3ŽP…ìx?6êKgÙ4?—¼u
^'{?‰üŸ€ìØ?ïûé³‡M?6AÐW?[Ì!b
M?,rñÓ?;[tðG©?3')ö8/ž?ïߋ°š3•?lC婰Ǘ?PDâáßY¯?Q!ÀŧJ?hQÝí*k1?eÄwŸcÿú?]ql¡?rÚþ)˜U#?xÀO±†.à?j{¤Ò?ô'Sä‹?i' ^†Q?ïÞ4š!º÷?a÷0Øæ€?D–ÛÔW7?·«>É7œ?p| ŽÒ'—?a½;,S²AGN3FGL J2321.2-6439@sځ¿½ð'ÀHç( 2:À:ªößÅÍÕÀ<	ø¶_¢þ?Ù+ÿY´H¿@'¨ÀSÓ@4ôBp¿é§ÇQ/?¿çªyW@¿Ùù¼ÚçB¿á>ãAAGNbcu?ïêzæ-Ïz?d´Gªïnl?<ia?¾ÕÙ?Ds%ä®æ?a÷í®äð]?bKf³ÐÀå?ï=®áCk?–¦îXó/?v
ԝß?"áç6¥m?'Ê~ª%?»êAöÇ'?îEÓ|ÇÚ?'°Åådäª?'ÀÚD<lƒ?'e?–‰Â?¢OU¤]~?‹™Ð!ö1æ?î¿û§+?•¼9]˜?pÍÑä¢^?rMH!r¼™?¡ôõ6­¤?"¤FÛV‰l?ïø½é°o?D|ó|1F?'6_4‡[?$¥@õiuq?G:Âml"5?Aäë'Õ
?ïγ܈N?r.ÌI®Å‡?XÞþìBR?WQÀǦ?rnR!Ä£™?l¿'Pûë%?ï]> «?zëÇc×?í?€4Þ%‡?t83Zšà&?ˆ!E¯hŒ&?o¶
>"&É?ï»<JDX?rŸè²kU™?eùªÑ§^s?[xû:Z±?weZ3Z|?o2åÕ®/AGN3FGL J2321.6+4438@Z¤[0HÀ.»›>µGuÀ:ýþž1À;ºÏ' =¿ÚRqÿn,%@k¢Câ-@ÿYfú¿ç¯3ëáæ¿ì8æv1Æ¿ÛId祿ïÿŽî½AGNfsrq?ïíAš\À©?i…nÉG@`?8Ñęà?;@»2÷?_H…kîrZ?g¾'Ö.'?îYk-lí?ª*íòåF?ŽÅÖéüË?'Ð-,óy?¢¸¶æL?¤Á
çIOÕ?ìÕqìÑO?¡ŽþÚíË?¤çæt`?SݤüÈ?®˜'Lv¯?œ;ìÍð¤?îÊø¿Íi?–8û™õÒ?|Í'ف©?{URÐl?¬	¯ñÓÁ?œ›G|gñ?ïôur?Yÿ?Tïæç·?4¿B+»É?5de‹ûù?QåK8†¤?RB2øÎO?ïuÉúE½
?\ÙßTÅÇ?tƒ~:s#?rwB+ɇs?ˆKÂ'*±ò?‰	3Ò·¿Â?îeQª?'8°óáÎ?˜J­s!R?€ =»ŒŽ?›7'Ökbù?ŽÉќt¨9?ïˆûî'38?yÀºšÆw?gä?YÛW?]3Cà
Ì?‡Çô'[o?v‡~\	½AGN3FGL J2321.9+2732@Xêãÿï9À?A§¿Í
	À9bCá× 
À;¢d¾£À	/]k!Ð@Hÿnàˆk@BPàW`¿å']竏)¿â's%Ui¿ã˜|+RFÒ¿â	&I{RAGNfsrq?ïW'ú‹C?—‡iŠ?`@›sX¢?\§á	íD?"zKܳ†?–'sãç"?ï'fó»4Z?Žß'Ã=ì?lK£kyPœ?~Þ?sWð?ˆSZA«K<?"ü"u#~Æ?íÖi;qµ?–ã¼oµÚ?™Ö\!üŇ?…¢Jk~Á6?¥²ë\&hí?Šº›¬JJ?ïnµZ?f?ªwæ«?¿Ç¥]?6·l5+à?'•©WÏ5?óÃTÕ¥?ïÚ;EƒöM?sꜺ5"?Dÿèo/"P?@|'?ð‹/?pB` ËØS?s(ãÀK6?ïÕkrÐé"?{3û/幖?VyDû_ÄÐ?fD¾Uý–Ñ?oWêy
c'?q7u"D
4?ïL¢VÆO?z%rk	h?ƒipŒ#6?pC9g_?‰mùŸ¸A?m¨Ã9šeO?ïâVLùéø?i|dîÔ\>ҟºE'¥ó>áFÝ£^ˆ?m bäŽMù?iwõe`l¨AGN3FGL J2321.9+3204@YkìAÝ"À;àÿ‰¸{À8«ˆTüÀ;j´MzV?öØïæ|,@9DQáõ@,n;òÊb¿Ø›£¯¿ä%:cËxÜ¿ä˜1&éxÕ¿é,ÛGÁœAGNfsrq?ïæÚE—u
?c©sÒÔ+?ZËÄ%"¨.?^Ê¬ÄÁ&?W°5N­Ã?Ofôèùb?ï~Í|p>?ŠàUA…Cg?mé
£ýŠ­?tۀþÇã…?ˆÒ^]ãå?"§3÷X…‹?ìˆvmçÜj?¨óßÓh1?°'ž£è©¬?¡ÒáD=0?¦S[ØÔÿ?™IywŽw•?ï²3M'{?ƒo꧈ڂ?Q%}B>÷‰?a·Î‰Í‹?N‹nR?'aÌz0?ïôs®M†?OÌbêUl/?MJ—ÚÚºÕ?HI'"]‡?B?™Éd–?7­¯ŽŽFú?ïÒ:<'Ö­?qH9P‹¿?XMª?0?T®Ç8Æ>?pÏw4…?lrlSšAÄ?îtI"*CÃ?™J_Ÿ¢È?ŸB»Ôf{?"¢í©†ä›?'4èڞ?‡K›s‰E¬?ïï"ßÇâ?a1*¥´?E™ù°&%Ñ?Dœï±-7—?VíáÜ\Är?]¸ÝŽ\jâAGN3FGL J2322.5+3436@Y·ÃŸý`éÀ8ÇóÀVœÅÀ9þæªÄdHÀ;v zÉʺ?çS¬#xÄÒ@"DvÒoN?÷­ µT?Ñi-竹¿êAb7­–¿ÐE­e¡¿'ãžSbAGNbll?ïL_:^\?¤öÍxJ?9"ÀÏýî?AŒ=QéËß?Ÿ'ëû;J.?¤çgF¤îÑ?ï9B"Y?5«<íÖ?v'è!ô	?€¨)Zénè?"6óÿþ?—£pvÏY?íóôÿú?™Õ›H2ƒ<?"ÿ웎ì?ˆò:Æt—?¦Àȳg¿æ?"%'þÓVÀ?ë5rTJõ?µ®õâ1óI?uØ°ï@Q?ŠMt´E?Â{q',C?µÖt"Ðù?ïŒ 7À?˜Á7 Þºé?@äx<ÑÆ?hŒ)ûnNQ?‹éªÁÀj?–œ1ý½«S?ï¹Äڐï?†i¾¼g­?c0}ùm{?s?æ¡ìm·?y…ŠŒ?!×?}½¡ éÿ?îä‹	ÞÑ?"_ÉêcÔ?Œú [û›?ˆ"$€*[?"ñNš}e?Š--³ã		?î¶jp¶Ä?"7Gf‡M±?u×»BÎ?{Ӝ¼è?¡÷……5k?'ønö‰²çAGN3FGL J2322.9-4917@tè¶@c^ÀOÏ`%ÆÀ9Ïûf=K»À;¨Ø+¥ 8?æD`ؐ'ø@lõÌ ?ÿPý Q¯?ïýÆÖØX5¿à'ÞIvìq¿ß̃ˆ©¿âOuiõ£AAGNbcu?ï¸wdTW4?z'5·9˜?V^s?Qišuÿ
?~ ö&ƒ¾Ž?xQ–
þû?î"0´†Ê?ªõµ¢ Â?Œ–Fzy?œÈ5ñv?Ÿk²NÈð1?¡zzà¢?îúY¼£¤?˜xÿ‰ý3?"ÉAˆþš9?'"ðŸÐ?¤»¹ '_¨?'šìVµ+a?瞡«-b0?·S˕Pp?ª$êàç•?Ÿ/à…uÒ?ÊüsX'=Z?µÂ[\Vžñ?ïãX§-xV?g©Q$ç<N?AàÙè/j?@ä0*v§?h/W‡)˜=?eh«ÿ~?ï|C~É£f?'IÓ§•,c?u4­^'ú>?}Qß½]£?†TɟµE?‰n¨`J²?ï;xî:?…Í[‰$ ?–…ó‰vú?pî;`?0?‹rˊ¾œ?ƒ"
®ýΉ?í+FrU2?Ÿ)
54Ð?œÏ*'T?"ýßí¥…A?®äÉg˜?›B²f òAGN3FGL J2323.4+5849@[ïÆÁ#À3€5'À7Á»øi3À:™MüUy?þœlâ×P@
†"Gwã¼?ñ'‹h(ˆ_?ïÿeÛüëy¿Ë¢:§ñ¡¿Øh|U»ô7¿á—"¤%OTHERsnr?´znÀƒç?µ.9ÿ·"?æámaÚ?˵ì""?Ês¾<nÏ?ǔº¦s`?góT
Ü×?ƃ Yl?áì><P¾4?ÆiA;xjå?Û÷œßtDK?ƀ¼Íjj?ÑÊÄæh¢?²"%ñ&)}?ÔrZ‰þ	õ?´8ò<ða­?ÙÂá`i?µ,ëØæ?ªè,h'+?Ÿ9ub?àîæ=?Ñ?ԃ€ä¨?ÚÅ-Xu.x?°Õ¥ç?ª1t¾¯,ó?±@Þ)›?éŠ4¸T«å?ÇÙ¥Ã¢'?ÃJÏî%ž0?Äæ›Ó¹-¼?x€Y¼¿Ðn?"ê«`êœ?ã鵔ˆ?Â>y¢Ù3c?×ʓo'ê?Âe30g?ÓÚ2«ÎÐ]?²}ä爫Y?Ù1˜5bÚ¸?´ou¯÷­`?Òô5á5©?±ϝ4úK?²k·Ä{:?œÓ®pô½_?ä'pØU—?µ~ÙZuà?ÒB[8y²ã?´
Ô?b	˜MIXED3FGL J2323.5-0315@Sr‹`òËÀM@TƒæÀ8,ë-
$FÀ;K_Û1ê^?õðÚmÊ2ê@©8<²bé@}8ßðk¿ßû²WDy¿åÖhãªp¿äƒcþ"T—¿éN,™¢9AGNfsrq?ïí¿Gö[3?\Òº'?P­Yš"+?SðŒþ×:'?SÔ`^ùVa?P9äݬw+?ï'ó·3T?ŒÆw»Pã?gϤD~ó?{ðߦñ'i?…OLÚ©MO?"k•H}Ò?î$ ÕG?–eد«•?•äÁ´`‡d?‹• ~žÃ.?˜6ªLtkÅ?+÷.ê?ï)4u:Œ?•ÝOkî?cðmpnÇ?oÛ'&·.=?˜[lfÿª?•,뱌9?ïöl֗ü¶?MVÍ®ÅÑN?Eñ"ȸ—Ò?EøÖZDc?@['šÛn°?63	Ñ3Ø?ïÕ{F"±J?q2ïÍÍÂ?VŀçiÜ?TÚ_~3e?ozÖÑV¡?k	`BŠ:?ïAwrìöR?†d,OiIÆ?‰–E@ÜË?}C_NÈ?†Ýó'Ü?w9©Æï²e?ïÔ«[
ê?pÙä¨*¿é?Tâù+õ"?Pcö¼`Ì$?pq"-þ!Ð?o
"BÆAGN3FGL J2323.9+4211@Z"º@Ù$À1Îÿ:cÀ8—nVõ°À;&Lké]&?Ñ32á0:@òÏ1+7?þ3'€ù9½¿âVÊÚóñ¿Û6fã}­¿Ü?_|ùa¿Õ¬HßÂÉAGNbll?ïü¤£¸×M?Dgbœ*²?¸Fk*Q?K€žV[?7C×ãYÀ¶?Còî9D?¦?ïjá½A5ø?v,š!ZÂ?q05˜aaú?vU€~*Sl?Œ¯uå9Ÿ?Šê
no©™?ï?f-A¾?"?.å€Ù?/ä¦]¤?råúQ¡p?v˜ø.Ü?€$q£U5?ï"vp…à:?‰J—«?Bt†GM?BkÃÁiØÆ?› ŽFÓnÀ?ˆÖþkúÉ?ïÊ´G®ž?²™ŠÇÚú¬?JòÚ+*oä?'Í53-Ì?wGœÈJV?°jä 6½h?ïƟùý[?x*œTk?]ZñЫÁ?Xx«H©Î+?uoìÉ*ό?tð:¤'y?ï¢Ç>dâ?s¸UêhÏ,?t2µ÷؛
?hžx»"Œd?zÁfjTË÷?kÈm—ˆo?ïÇEþ3o?fÇ6AþÑ?9¿zå?)ü˜Üªú?zÕëPèÈ"?fH7Tg¤ÂAGN3FGL J2324.7-4040@uãV¿Ê…ËÀPå}ßÿ¯xÀ8´@éÕPÀ;
®J*Æ?ë<¶ÅrÍ@
Å6ϟåä?ü*@›P©¿æ•¡%ª	¿Ó~ÉDé$¿ÕN›}ÁÄ¿Ô],bAGNbll?î8‹úbT?§"iJo°?<ر†*?z-éØݺ?¨(q©ÿ?¦-)LH&?îèÔ~¶®?§Ñfm$ú?'í–_j+<?™+¯µp3?™n¤ü¸È•?ÆD Øx?êtNy"Gy?ª÷k\ÊzE?­™e£:0?˜W€¹[¨?½•?~r'?¥¬ëÖ´Iw?ãeâñÒ@?¼1!WŠø¹?šæ²Wÿ»ú?›.¡¢ki?ׇw€âá?¼g&ˆ]±?î¨óX¸å?¡#ãveæ?w²ð&÷?zMl¬êñÞ?¡ÂÞhSò?ŸO'S"Ã?ï—p"ö>?'´ˆgªúŽ?qgxæ—ãZ?'Ú	&<{A?p"y?",+ùITÍ?íšysQ?›ƒF¡ª?Ÿ/‹Ý%—?Œˆ_óK4Þ?¦À¨Ù+?'ó¢(Ó@¬?éWÑ~_?­·sìƒC?Ÿ"ÍD•&?ŒÞs''Ò?Æ°8Œ¹a`?­AôfÂßAGN3FGL J2324.7+0801@VA©¿ìêzÀH†|à%o%À9];÷'À;*Ž:Á¿úÖMI^î£@/Ø;Ù@5æzyC¿ÄT‰ Žfœ¿æ¶à'>祿ÝQ"	ve¿àGBAGNbll?ïö³"?ãE?PÃncdÆ*?!Ä¿T×£? *+Œõ– ?P`A"V@4?Ou>‡"J?óqÒ*?'¦›'Ϭ?d8M?en6K6ü>?""u"+?~/Ꮇ¨¢?ï4¹‹…w?"r¼¶VJ.?Ú´ŒÿR?sç֎¥žW?{tCŒr?€ËYIP…?ï†]Xs?']ÂMvç!?
MåRæÊ? R÷ĸ?Ž`ÚßÄì?'Q#¨¸…Â?ïûgf/x­??{Q¿ÕÇõ?!ÖåUyYy??
"‡ì?;Ù[H[65?;‹íª;±¥?ïÞQ{a?l²îòÁôò?PcUxw?Q:R¾?i|Ùïóáð?fª£ù¸ô?路æœèÀ?qÔ2Í'Õ£?r÷:˜žo?aü*hÍ^™?z­áý®?l:uÒ¬?ïçß{ŒN"?Y+LÉÚž>èÚª·÷×>èsJòl€å?hªF´f?YÎèj'AGN3FGL J2325.2+3957@Z`u>p~À3ûý€É¾ûÀ8ñ?Ãdn?À;^>¢‹±?øž|DŸ[@—ò'OOI?øœcÎ[˜?ÇñÃ.ñã¿àzµäå¿Þ´3ôNF	¿å¾ÄŒó$AGNbll?ïn~'‰T?¢×Su?Xñ'm».?aԔ'yéì?¡¥-Øs?¡"eŠäÄ?ï+Úg? ŒƒJfš?é@î+?·nG¯Œ¸?•×ŠuLMÛ?œ¥•oK8ú?åÝÙCA?º¨©Ènw?¯‹jÏ#?®bQ¤z'¯?ÆnëgŽüÕ?µ7å
x'\?îboÆÙ? Û²'nÊ?€›£w/Ç?|wÑeÀP¡?¥¯@N="z?Ÿ¦ÄíˆÃ®?î$°ãQ|?ǁ`d«?'Hõ8
)?µUêÃ,åç?©"´zuü?Å@joEÄA?ïŸð–ß?‡À'ùÿ?k‹ø	Ô!¥?düŒ­øÌ/?[…ÞŽÁ?ƒ°è[ñ²Ó?è8azï5?´L\sî?¿ªóþ?¨ÉZÂèI4?¾"¤xY?­ñÖ`c1?ïgכ™	b?"¡$<C•?À‰¶å<U?s5`¯AT?"Ih¯Á?q܊[Ã]AGN3FGL J2325.3-3557?ý"YßDs¢ÀQmœýç!À8¾¨C€ˆQÀ;‹³ünñ?üÑÞú¡Ç;@­¶Ð·?þ'Ø	kä¿Ö¸§'(¿ãpPJU¿äÉHROX¿ïÿæNËaŠAGNfsrq?ëâOˆ©\?¿ü:ö"è?¯5µä:î?´Íjœ<?±Tš'/J˜?µ=×R?¬"•p?²B»A9O?‹—Êqø?¡î‹»ïá£?Ýéñ?¤£Ù£õ¾?â}šY òX?´LçM!^?ӋRÝ%=/?±3ÊOŠzï?½åáÆ®û?§-,숄?îCnò‹¤?¥Tsÿ#?"<V°Vm¢?—ø+Í
?¡ªå'Œrü?ŸÒ°véð?ìƶPg)8?ÁþÙêÙä?¡ƒ­Û+F?©43–þL?±F¦G ?½}& —~{?ï4 Az/?Ÿw'%_?ƒwë™ÍŽA?ŽæÔR*®Ð?€e!U?"c™ô¶µ?âüÞ'7?²øIu'g÷?Ô² œÿ:ï?°ìHbŽM]?¼½–›Yډ?¥ˆf1?ïgä¡Õ¨?Š¶öæjœp?‡þFCƒ?{æ;
A"?~NŸ©lå?ƒ`ÞAGN3FGL J2325.4-4758@tÿ¹ÿÖ•ÀO¡ƒ_›q
À8÷.=*,úÀ;wv¡G
¿ÂÌV|°Í@CDÁ{
@|| 9›Ø¿â®Øê,¿éêï¼TÉ¿àŠj%™í¿Þh¶ª÷eAGNbll?ïøï&WÇV?HÛ6ñ5?îió U?^žI?H¥™D¾ÒÛ?FtYÙ­?ï—OÇu?‹¿À"Y?fxöÚéû?|ÎÌvN²‰?"«/÷
 ?E¹¾ï;Ò?îæ"Ü&˜+?‰ß'É·0¾?"Ã0®Ø÷Ò?pFGç
(|?˜Ëì#À~ª?†6éì°Qs?îˑâ§:Ó?"Éٞ›?@58g Ž?@.5Yï?£Üÿ7Á?"¹¹Ï¸ó#?ïý"A1'c?.¿ƒïÞ.…?z"whÉ?/ó.IÛ_?/~¦màèN?*꽎f"?ïÝÄû-n‰?k…þü±¬4?Nî	/}§u?MB4®yø?j'¢uK?fã,™á½?_ =g?pÕl³þcä?swäÏã+®?Ya¤'†g?[õ¢@ œ?k#%=	?ïÁ
x÷/?kŒU§²?/‰ÇºJ[q?"öpì¥W·?~~uacË?kVÐàòbwAGN3FGL J2325.6+1650@Wɪàú¯ÀD®ö@c^À:02ˆéH.À;ÙÏsëŠ?ҏ‹Ž>Å@ÎÙçè\@Ï\ÿµWe¿×C[Òí*ï¿â.¼Á'ۿߊ‰|§+º¿Ü	¯j«qAGNbll?ïûî¢×Ó3?3Ûlú?˜[>=
?ðËð£‰?<dТ¹åª?2‡"úcj?»œßÛ?‰ÒΞ1z?g¤7ËÔðT?ržŽ7q'?ˆíÃÛï#?"{¡¸¬AX?ïSÉOXœ"?€HWÝ䃗?€³M½u³?t]TC¢
?ŠZ–ÒÔs–?t{§öf"®?ï^Ôt[?††O#?T½Þ?4w?U¯—÷ü¦?'óMñ4?…uu*­e?ïýåL[´m?!ÁîøEÌh?O€Ïϓ>ûª¨ÙÞûý?+ãgf¯ƒ?:\oRM—?ïÕk{5?o O‰1ÄØ?UNö…m'?PÖ8?¡¤?p,·?:1?j­<uéqŒ?ï¯éO—ö_?l'7 çÏÝ?q6Œ÷x?`‰î]Ş?vÔº¦]c?e&=|Cd²?ïßb,´­¶?a±W‰}d~?GÖ@T$ ?:–×ö?j¨Bý÷)Q?`g7ôBpAGN3FGL J2327.7+0941@VÎ]ÿú÷ƒÀGûæ Zé[À8sþk«IÅÀ;Sï«&\?êê+žQ @uiäu5@lÆ 5T¡¿ç',ÐÔªx¿çž¯rô¿/¿ìûXùé¿ÔHæ"¥AGNfsrq?ïø
bÚjÅ?Wxc™À€?J –OS12?V›" †Ú?&×w¨d^À?(ji‰^kÇ?ïœe¨j0º?ƒeCNLÉ?aŽ@€âS?cïÿcñ>¹?"ƒÔ6jÏ?€![Ì,ßt?î8Fà[—M?•cLây	ì?"ý5p0[ì?‡¡'Žh¢§?¢|÷ARv>?'!eÆÕÓ?ïÙ)ðqö?tDh–í™Ø? º3¥í?(Ò½"²?s"ö©§õ?túû+í?ïûëÙàå?BôQ¿¿,?4Ïbšå¿·?<˜C~2?'£›0~†?*xY^ñ?ïÜD¨ÀAé?l&ý4i?RN3À§õ…?QGÌVŠG?j"=>mܤ?e|/^9·?ï!}~0?Ž"Ò¸Þ©$?Šgéää?|ÃO>Y?'±œ†
>»?‡Ûðï%n"?ïù¬V5×?Tz_`óhÎ?z¦Óc?]ké?H,ð¦àú•?T-ïB«¿AGN3FGL J2328.4-4034@u×TߋrÀQJërªÀ8r2$?ziÀ;M=5´Ã?ï¹+è'#~@Ïz>üë@wö?ŒÝɿݵÓ€ná¿çñ@/׿ã¥'¹ßü¿ç{$Ö³šAGNbcu?ïû
ùš?8–ÆY?+Gœ°Ô?*^eÙ7ö?9ð8b¢?2EÀÅÍãD?ï¦p&و?…=­Á‹ÿ?a
+ÍK‡?c‡g?º¸?'!k`ÿOÓ?I
û·?îÛ¿$S؀?Œq)|¿Ýë?Š›íL?zšQ­£8?—:$ï±o?…ÎË×8Éf?ï˜,ue?†EZÈaà?: F›"
?Lö? ¸Ÿ?‰àd!?…î
'³©ï?ïý"5µ!=?'cE¹,³?bɉX|A?ǓÊ×ï?'@L4¯µ?Çi¾ðÕð?ïàç`nL0?kh;ê?ON¤ä¿OC?Qù¹Ì3Y¨?gDöy£jã?d}†®_˜?ïx–Ëo:Ý?xå÷×l¬ß?}eFF±x\?l"¹%暄?ƒ'©ðZlÇ?qŽ¦}V¿?ïêw꿞]?cŠ¢¤eëŽ?1â¹\?.vœ¢â?cUøÏCþg?bÎ_æltAGN3FGL J2329.2+3754@Zb'!%¶À6*ÅÑqwÀ9^'åp1ÁÀ;rùÒ¿U¿±Ž7°ñO
@Êt[òo?þÖϟåãõ¿ÚY^ÅLÄ¿æèϼý]¿ÓœÎùÁ¢¿ÉËV=ô?AGNbll?ïôsL}Üû?H¥6¼9!?.U
͟aþ?&Úìnìº?SNÅ­˜,ô?FuR|à"?ïjÖ\1s?"æi\ä'I?p†Ýë8ä?|Ž20G|1?\þž?´Ù+£ôq?îöÛmñÂr?†VYL#Nw?†uÍ}Ê?sÕՀkÈk?•é«†ªIW?€£¾Þ½1?î‰JóÝ÷†?"8~­¢=—?Dø[Õ?L]0%Öõ?§oR0??"'ùP*¾?ïú~É0õ?5M;ó¶?%^#ÙµÂ?萓u&…?@­SÞáÛ?1'd"ÚG¼?ïÑ%IÆ?r•N	éö?V¥DYえ?R}Îç¡ã?qÄ+£§Ñt?pŸ`óÿ?ï‰ úîÀŠ?q—j'Šyž?xL2"ñùá?bçç¡&8?'¨íF?i|¬Ýó؁?ï±ú
óy	?l»Ë¦é¯£?8ñ§ûˆ ?/z§u?'¹ðN×á?l^íϐq^AGN3FGL J2329.3-4955@tÀ@%NÀO(?ßéàÀ6¢áÌ8RWÀ:Ë%Ü2›@Ñ´d ;	@ ft"§lk@…ž†"W‹¿à®•ó­óT¿äâSþô¿æ|ÖJ­€à¿ê(…	¿œAGNfsrq?ï·Ñyɉe?{Ô^p1™?qnQóaéÙ?s.}ï(?r¨ñ;3r?p¾©¹è?ï§CHݝ?‹	É¿0"?b€ãm·¹K?z´ïõìŒÎ?Žôùá]Ì?'Ÿ‹[ ]+?ê²QEM³?¬ïÛOßuÎ?»0ÄηÅ?§ޛÌç´?®z¾FKS?¡ªnK^¹y?ïìr÷O?sž+–Û?!²P<).v?R—Mû®à?br½º¥ ?rñçß®?ï¸qU2À?«Ê m`e!?c,$ðU?hÝ ›Œ?z12- áZ?«ÃšµR¦¤?ïá"V	?m¤ð‡3ˆ?NŠøij?Q_ÖC‰è°?g9‡f¸Z?føÊj"ô?ë×b5ûz?­¢­÷A?¶æ»¶¼úy?§YvÝø†?¤¼e@^…k?Ì³X˜v?ïü*È*&?R|ŠÃ$œ?bR¬Ìl?‡pÖ2X·?;¿AÈKäZ?Q­Vøý²¿AGN3FGL J2329.9-4734@t÷:ÿ°NèÀP_¿î—ùÀ:*Jmâ\À;½êi•ÅÐÀq—:ï•$@Á3¼p@Úf€'ŒŠ¿ãýß-;f¿Ü•AþÓ¿è÷%L¯tç¿Ë™ˆ/lˆAGNfsrq?ïåK R!?g^YèÙ¼­?UÔ@Ê ¦8?[§½DSÌó?_•.ºw¾?]<qÄj2?ï¢É/Ö©½?Ši±P~ú?c6°ñòòŒ?{YÉ~õ?'€Í(è,?`³Xl?înþÀ1UZ?'Qœ™˜à?•;Ì£ óD?"x(Fh?œä[Q÷…?†»¦΋À?ï¬
EºZ–?€Ì1Gæ?þ˜ãþ?î'EâÊA?"êi"…?€‡àôsó(?ïô±ší+½?S‡È#VYœ?Bï¦O—-?GD²oØ0?JIíµ['?I´T'æ$è?ïáÛh·œ?i±ÏDZ5"?N³	k?Ps<͍ª?fŸ;~"?c]1'L?ïX‰û«C?VáÎe¢ø?…Á=Spá?zˆ¡ˆÖÔ?"Lùтi?k}Ô=mÂ{?ïñ•	ÖC?RôÐ1;Mg>ËàOB§Ü>˛ê¯Fý?\ÇӀՄU?Rñ…KSozAGN3FGL J2330.4-3726@vJÓß°Õ ÀQ"ÓÀíÀ:TX¸þ¹¯À;öBzÎÓ7¿à²$'( @*éÓmо@Ž€¢§µ¿ã/Bóçæ¿ã8ßi nÏ¿æȹz¿áÁÁ¯@—AGNbll?ïèÀ"–`»?b'¤î;»?E}µ«>Q?FЄ'üTù?aßý¿P'á?_î<
ÃQ?ï‡{8̋?Z{3˜î?gŒ¬FՇs?yݲBõØ?ˆ>_gH?‡'!q¢?îx"üiÀ?'òe$×?'ûŸ5"?}Ä&?ĸð?žñÁb†>?ˆ}'®Ç0ß?îíÁzðÇ?']'•9?YÃv_?UvU*T–s? UÐWuü"?ÎÈ`½–4?ïøíàvUz?Eo¢z¯€?)z÷-¿{?%ݗŠG¯~?EéÁ=-pf?B"[Ó†?ïÜ{ö'æD?mR¥Ò׏´?P¬¤¿¹¨&?Qc·•%Ï?k-¶ä˜™?g5-«²?ïoUýW?tÒü@Ÿ®º?€aN²<>$?i»2˜v?ƒÉoČÎ?iËAþ™JÚ?ïÏiˆ•÷_?hZr©¡É?;üŸæ?,Ý	Ói¯?v™Ÿ•wL?g—ã ö'AGN3FGL J2330.5+1104@WD¶ŸÏ=ÀÀG†"`LpòÀ9¦5\_VÀ;‹võ)ã(?ÅÚ­Âè¿¿@|û£$ð@p¯Àw~è¿æV< Õ^¿çüŠ I¿é	¶™üã7¿àpý~ÎðœAGNfsrq?ïóHK1«?R~áО¢E?EM—F7º?DÉZµMz?M݆ÛÆà??GOªX÷dž?ï[ßFÌî?"•%oüS?n>œw¯?Á9!Q?¼Sùirf?±4ñJò?îØ%RõÆ@?ˆbå'Œ‹ê?‰m^"Ž[±?t(ûêü?˜D¦Tn$?'¹×'ÊÄg?í O\Dà–?šö÷BÂp?v»¯Û²¾8?r˜cÔf?±'Ê"""ª?š 8Ë÷°h?ïú-`5t×?='ìƒöÈ?2Á»-1vN?.Ó綼Ç?;ÓBe¤9Á?3Å&ó=ò2?ï̲"2ei?t=ç[™Y?WIpq5,?TQ!?F»?sÔa¹Qô€?q"yŒ‰ìÍ?{ð?sK;!a?wòi´b"h?g²G£ 32?€ l)Ès?m*±ÍæP?ïs´;ß?{¾Åxq¸?b^󜗕P?Rq1Eõ9?Ž{A€-*é?z34¼žwAGN3FGL J2330.8-2144@FtqŸÀQº ÒH7À8é¦W>À;'<b†ÝÕ?õ" pãÂÞ@±±Bؗ±@(‰‰V*"¿á‹³¾¥¿æ]'O7¿æ,‡JÀ J¿íÔo6"nAGNfsrq?ï·k*Á?rÑ8" ˆ?r<ÉîKѨ?p'Ѧ?YþvÀ7P?R5ÓÆðû?ôúún?‰å,և?f®Õã›I3?m'2õy×ñ?†'
FJÎA?"ò¼u'§ˆ?퀱ßÇ·u?žR#f!ø?«ºPë¢G`?˜EpGqËÎ?˜u"*œ?‰šc·î?ï'9•í?ˆý»kÌ7ï?ajðÿF?gCzEÓ?‡*žãP4?‡Þm©¾º?ïØ6Í>=?lH"&é§è?p+SÎÝÁ?i¼'o	è?Op•w­?E ñށø?ï҉¶ôH?r4þ<˜ûý?YÛ­gc/à?Y^'ë8î?pD3lY;¦?jÈdÌ £?î7£•ú[Y?•,{lô$?¤e©6¡{?'²cêá	ñ?@:ÐÜ?€JUŒ@?ïãö>Á²?p"¯MU¶O?QF"DWþ±?M0€gBùU?cf¬³¯öÏ?neå
CAGN3FGL J2334.1+0732@VôªŸæºµÀIM]߯' À9P>±·!À;œ‰çÒ¿¿K\¹ƒ2¿@*^%$QÄ@	À¿£C'¿å"«ÂªÎº¿èRk);/¿ëŠwV	L¿°qÀ•9–,AGNfsrq?ïåØ-öTÓ?n\'Á$?J=Ì¡.X?N"žKÝe?c˜^Ⱥž?k²ô"Õû ?ïb/ƒŒx/?©·Ï¾Þfl?jM»Q_Ñ?|åðF8ó`?p]x:« ?§àè±±r¼?îçÇ7a–?†¦VӉ?ŠB['"R½?y»]šL?•ü9Q#kç?€¼·äá?ïhfé?–e®›v??L•-°@Lw?WÈ}f.ú?ž:ɋ–úí?–Aª«uö8?ïój_30?Z·"Yï¶?A+²Ú¥oV?L
ØGã½L?P•h®Qxú?UÒñTm¢?ïÕ'!µø?z2ZâKÿ?S‡³ÚäÅÃ?W²a£!ò?pŠ'RÅ?vTe;OØ¢?ï€xR¥·?w…w Î?{±¶Œ¸›?pñ\Õ ?'	 ë&?möÊÌu?ïÕc+b?qLy¼Â±?&å½{ã?'s–¥Ó&t?t—H–ÿ®Ê?qçïnAGN3FGL J2334.8+1432@X$՟Ú%{ÀF0•ÿ±%§À8èºÅcLÀ;<
MzÝ?ó
…örc@CÒÏÆ&j?þ
j¬¾d?äh—ë»ò¬¿Üƒm
¢ùÈ¿Û»ì,
þ¿àÈT˜ÉAGNbll?ïû
ïÏ'½?>^5¨Ä(2?#™#f&?Mi6B'?=È3"Jj?9bN3›²?ï\¶tú0'?'ÄFi¼tJ?kúu')hÿ?kƒ»VšÐØ?éâ«]Ë?'Â{~ë1?îAF\ìÑ5?šËÑX¥?˜(­‡Ýæm?Õ¸3Á?Ÿ®†Ý÷Žå?"Ó=^˜,U?íyH…È?¨¿"Y
?~•>¦èçR?{qÑ^@úß?µ'áÑ~¨Ì?§TÚq×Üì?ïý‡yJ]‹?&'q¢£´?Ø;¶|Ì?H>ØQë?)I9þç«?÷hM}ñë?ïÅQФ•?ySñúòºž?\/Ò±?W)+Ó—?vKVV­œ?uÓÑû(4?ï½YÅ̱?Š¯'ð¬&Ä?ÆÖ¤ÎW?ƒ×hٞ?ŠÉÒæO&o?ää¡ÏÐè?ïüzSG?ŠիȺ&?yaª€?h"/;'?–¼XPó_?ˆdÍ»Þ]±AGN3FGL J2335.1-0133@U
>?Ö¯¥ÀMGy`>.9À9çÜÓ«
_À;–a(	4?äÔºŠˆ@)\šµ£@°Jߢ<€¿á|8xóÌ¿çlmiÃp¶¿åd*eÈö¿îáõrª¹ÊAGNfsrq?ïã'°ƒb?hŒpŒh,\?[ãM|;Ž?bBbJ¬ÝR?\ú‹5û|õ?W<b[:Ëo?î®Ö1%Î?Ÿ†Ý%ö¹Ï?‡VZE>û?‡h¯ŽDô?žz<c2ª?˜Ùâ	
Œ?î—Léhë?'Xz—*;ƒ?™ð9ÿÏ/?ˆ‹G­yÜv?"rŸCw…?ÖJ~|P?ꝜQɐ?ª×àò¶¥Ë?£Æ–^ɏ?"€³®=¡"?À—é":^î?§²ŒÊGD4?ïߌIœM ?"Ðç駱²?eýÓ¡ópS?"´ß]W¥Ø?TëÅÉo?PŠÁÈãbS?ïŽh.xÊ}?óèƃ¬¥?r¶1 ý?l‡w?æ?ƒdPÒ4$?{2±î¦¥?ï7FRʨ/?'v²iK?ŽÃö!ui»?yJ(dš€Â?ƒju9G[?s~¦ƒ^"?î<9ãaÊÜ?³G‹Fÿö?•!?Km?xG'=š_?¡«ÂG*†?ˆßI%¿ÅAGN3FGL J2336.5+2356@Ym¢£Y6ÀAê.Íû¡À:SefŒ&À;àø‰éù-¿Ôl£÷ì`;@
"yöf#K@ã_`bÁ¿éD~Lêœõ¿ãKä;m-D¿Ü4H‰()·¿Ô/X×*ÁAGNbcu?ï±ò×s?Ê–ýã:?fÎǝ;ÑD?Kwc¼?{Ÿ'ÉÈÚ?y¬{èf'×?ïyhP?Š«¼	o»?g|'Ö¤5?dÔàe²–©?‹¾x'°BÞ?‡ˆwÂ:Ç?î;vE#?Žl#ˆ©?Œ¥MÔ±a?v褯ýR3? ÂõP­;?ˆ§¢TÌÄ?ï3Fb~¿?‡1Ÿ°#?KaÞÏ©*?PM9ÉÄ<'?˜¼$ºÈ³û?†­×¹Xß?îƋ×(	M?Ɗácwu?¢Ç,Èâ'Ã?Ɣ1¯½?Z¸ÇÕ<Ã?]…Æ0W?ïÓd
.£?o̸áÒ¨?Uh©ŠDw?RKqayê?póÏ3ô%?iÍyÒHFŸ?ïgBȸ§?v/ÙNc?|K}Ü?i†Huæê6?ˆ°gñ"Ç?põ¦UÙÂ?ïÚ<õ£?bìŽ?9ÌM¤Ýjƒ?1gû*?qZìøÎÍ?aÅoRù˜!AGN3FGL J2336.5-7620@sIÈ MÀCú‹ Z›À9Ü-$%y6À;ΞÚK:'ÀßU®dÎ@é¥J§Ä@¤2`Ov
¿áre¼â
¿åÕï°Hÿñ¿å
1÷Ž¿Ú‰N³A`sAGNbcu?ï{¿ñ?­@<"O?b>ÆD^ˆ?b"ã.–L?ŒŒÞzh3Ã?Ž÷%>g"›?±"™ª?†Ì¦mYÎ?f
(Ð`W'?r³€J^?†M	!÷‹?€€MD'¶?íâa'à?—"Ò47Y?–ýÔ¦jJ?'È͈çI@?¦[hH£8Ó?'ýÅ4ŸfZ?ï¢æläf?€ªUG'ã2?óqˆNDå?R‰½^€‡?‡*qY
×<?€¤¸è.Ÿ?ïÍ,_É¢?ƒ\‰ðœ½?MËš S?VùÒ À?u°X‰Ç?we5?ïÜXc¡î…?ko¨¦Ê&!?QJÓ¤áƒ	?P['Ç5»+?k2ƒa©%?e‹·¨Ö'?ïFŸ+s?|Á&ŸÕ´"?ƒl´F‹°?p¨;wD?Šë…»‹?tªÍ,ÈÓ?ïï'-t
?WÀñULø~>ÖË"FyÅ>æ»Új.ƒN?`ÍmSÞW?W»¡IòØqAGN3FGL J2336.5-4116@u˜`@|ÇÒÀQG8à^*À95±/¸TpÀ;¬r9€
?óÙ—ïun@Ô÷!'@ê?Ðz¿Ü…¹}(¿á0ýg¹œ¿égÄ^á"6¿ä©ÀkžVAGNfsrq?ïî¬Jm®Ò?^Ñýø
?V``­´ÂŒ?Y1ì:%?HŽu à?F¥Sϔ¯F?ï¢,&hc[?ˆÀ†!ՃN?c7ua|ÙÝ?rîqŸã?'§þ´ý?''Ǽ7k?í¢çˆ\QÝ?‹1Þ¾½?¤Gß-ƒŽ?•¾hš˜ÿ?¡Šƒ–ÁÛª?'ˆÝÿéÉ?ï´ ºÏc?çd¢ÛL?K÷ã@Þ$q?QëÝö6˜?8S/€?q—ÅžÔ?ïøáZð´?H°t‰žÇ?CeY=ܙ<?CÂ
/½Š ?8ŽA#!$=?2¦@Á)ÔÂ?ïàÌÔ¸J?lۇõ]1Û?MãšR¢Ž?PY§–…8|?gºh¯-?fØýŸ_üŸ?îâQG+žÐ?SŒ,Iñ?""¨ë‡}+?†¶æDïÒ?!.2tDÁ?"®¼Ï%X?ïò%Öö"½?`­µGÜuÕ?<$öú[Çð?@?ÃýTÛÎ?T«J¢¬?^‰IÄAGN3FGL J2338.1-0229@Uï¤hÀMâ'àÙìÀ8µçïhHÀ;n\Âxµô?à¥ß‰N.@sôI"qâ@÷®XëT¿ãæ!¦² •¿æÙ{ªD¿é"~‡øB¿äíëÅ­ÁAGNfsrq?ïøÉxb?Bìå|<•?5Ú(œo?1Ô"q@Õ%?BR0¦¸ÂÁ?;"zÞ(xõ?ïR¨eÜ ?ˆm"ã´å?c*xvα[?d¬ReöÒv?‡`·Òt"?…¨8Ïǁs?îËa£ðì?‰ö¶óˆë?ŠÜ¼¹âÃ?v•Ãnÿºÿ?™%ÄÀy.?….ë˜x?îʃ·/+½?˜É#Õ/7?cb¤Ææ‡H?aÜ+«¨?¢!š>ç
Ä?—¬r	Y[?ïüøÜu6c?0æB')ð?"Euó6Qˆ?ùd§°0??.,Àw©y?&ê**ºCò?ïݾ¿lQ?iò«ð?P©`|¡?OÝ:Õ/ ü?iìÖNJ?d§"S@±+?Ʒ4	?v»
©‡Š?zk™ä²?i&Ð$vQ?'f[³¦©?pß^!®Þs?ï½ïÞ¹x ?wVø¨|o??J&N]D??£,q´õ?}ÃFÁþc-?vÑ 8@£ˆAGN3FGL J2338.7-7401@sYPà"'ÀE%àdYFÀ9ʝ}SèµÀ;¦¶Iӈ©À@2¯´ì@Mlr¹±?þ4¢ÿžÜ$¿åÛá"ÒVò¿ãkܬ¿â¿Ê[ý!(n´¿ß˜Ëe;˜AGNbcu?ïýî0'n?.̇ð1Pd>ñŒg‰È_ý>î€uibV?5÷Ȟ¨ ?.jÄk-%?ï›r$	ʄ?ƒD·|ES?bŒÔå–"?cô™Æbò?"€AöóÑn?Œ|‹#µ?ïoÎü@NJ?{0. ?x†lÞ««?pY¢ÒãL?‡É
>æ‰?rÊò‰tÞ?ïù&£ò|Î?WÅTÕÀç>l¶*lÆj>—‹Àžsª?Kdþ:×Ï?WÅ)'J®?ïþ	F`óœ?1éñbm+?•j"^<?L˂
]?+AU(́?-™v"ƒŸ?ïÛ´ú¦­\?pÀ|ü—?R@ülž?RÆWKA ?k*†õ¨½<?k" ^Ð]
?ï¸hý£?m°C«"2?lÌa˜ýa?fù9¹Ëmp?uePd
R?aäc¢ªÏù?ïþןÊÇJ?)oó,ê¯>7+;ÆlcW>t5xnÙM?"…Ðéz]?)p
®ºðrAGN3FGL J2339.0+2122@YPyámmÂÀC5ëß·‹À9ãIŠÀ;Àaâs'¿œô
Oûp@ρó_³š@nԀu¿ååª	ºz ¿âÑOS'ç"¿áАDõí¿ØswšÚûþAGNbll?ï
~<W/x? ºzÀ´'N?T÷ż?R±Éõ*²?o'Q¾é©? …ÖŠY?ï!߆ÁXX?Ÿ¦fL3a?x'ó{˜íÄ?‡^t†?•Ÿ'L¶Kˆ?—…ÁGûÝ?í~TQ;?šÞ‡Ã2?—$Ò=<ð?LeÞL?¬ˆQÍÇ'?•©—–ôž"?푏6¿.Ô?žA0ÐZ{?z7K°¬×?zŽî»«q?±ÐS`?=ò‡<7?ïÇéÎe¡?yã6½¡¡©?B
#Y»?BEވ=?y»QÏ|fÅ?xŽ‡¼ Ô?ïÀúño»Ç?|:Üê»	?_–£ÕX?b1DW00$?w»á©û?wt"í,|¬?ï:Á=ç0?}¹—¬R°†?'*(üë§?n³ê¦óŠ?%—dGC?u¶Ñ*-Ò?ïzë[á°½?vÙW‹wÌ?dž4K9ü?Tly9J¤?Œ§IŸJ!?uE«Ä/:AGN3FGL J2339.6-0533@TUGÀ'áÀO<OøÃÌÀ8:[Ê+1ÝÀ;MQN§-@M¹2;;•@
‡ûÐñI¯@=I#àYò¿Øú"¯-¿ÖßóÙ^´¿áÇívÝÏK¿ìm¯nJ¾ôPSRPSR?vj"+"ð?p²+ݐ«À?ï†Dqb݊?ˆUyÚ¤¤?ƒk®aK¥?'>"<h¥¬? Xéšö¬h?µ@Þg_ýÅ?ê&Prøß¿?ÊÇ}ájO?ÃPƒÎߪ(?ÅWk)wP?±/2 û³?¡?Ä ŠM?ëŒ*aÂ+£?ªðÎ7?²'}½'å¹?¡ñÝ-ª?›pçz¡QŒ?'
´|‹Ê?ëý)ÑW?®Àto€¥ß?¹;dÒ^ÿa?ª%Ö ­z?bõ}¸@…?eI¡Ì¨k˜?ïÅo½An?vµc«tX/?sÍb¥
îË?nfHU?­[8d9TN?ÁS•:a%?ê	H¿ v?Ë_	{"õ?À"çhHX?À8=ý¡½?½'9×DÓw?¦ÎŠ¢fäê?êO¬lÒ?­xåˆÊ-?¯âËïZªì? uìb¶¥æ?©§"¶*u?"®Zå·{î?ìa¯¢Öô?£Ã!5'?°Şo©?›Ó-Å0PSR3FGL J2340.7+8016@]öaՈ@1Ó8€z
ãÀ8Kê¸pvÀ;$'ÅA¾?ìhSbÊòÏ@Q\ÿ_q*?þ¦½žÜy"¿É
BÖ
Û¿àŸ@ŸNÜ©¿Ù-ûȇ»¿àPºAGNbll?ï°
ôVËá?yþÞIÑJ?y'>}y…?q!"jÎw?líŽx¨,4?kwå}¿f¼?ìU†dlÍ?Ãf¨q‰ì9?® 5ùÕS?³
"ö¥5?¬‡háD×?¹ŸíŠ1?í‰>¾u?ÏRîLiß? 7ø¬Þ÷›?ß¢þ¢PÛ?§4&Ç@Ñ?•×"»;ú?ä§]erè?·£®`øv?·µŸ>;?­–•ÈȔ?Ðé×ͺf ?µe"?£À?ïÑ©£Qÿ&?o¦ðjþ%?plϽ"3ø?i1êW§ÿ´?ZùzGtSÔ?V¢«Ï_¥?€‰'\?²Ð®4AŒN?š7ǜ«)¶?£(¸lü)?•"hPxÚ?§?kÁ=NI?î¯ÂÈ3'[?"Þîq3à?">"©ú8?…ØTY7m™?–É'{Äòc?Œ"ïëÈ«ú?ê¹ß¾RFÛ?£…{'H6?²Ú[,€Ï?•?ÒþÀù?¸'³‹"×?Ÿg°ð ¯AGN3FGL J2343.6+1551@YŸ'xÀEü_ !¸À:@µ¥8À;Ô+ç—r?éÿ»ä¬@´êÓ@Q¥ÿÙi"¿ä¶›Þuõ-¿ìårÐ×ôH¿àKcEŸœh¿åm{ 1ίAGNfsrq?ïõPÐä?Yzž‰b?%QÇ6?,©Å™æö?S8´±¾Ê?WÈÐw©ë.?ïêó±ñˆ?˜ˆÑd%e?yê^¦Ô°?¬—¾œ43?–ˆ	åŒ*S?"' ]÷
?î%°¬¼Y?"㜣ãj5?'Í:ûÐ'?ƒ¶­‰b*G?¤¾a&Åî`?¥Üaéu?í¥ð%R±?£ø¥@1l‹?‰²ËOäÒ?ˆ‹EUD?¯4Jåurð?¡²"ePSå?ïúwòÍ3ò?GŽº™ïÐ?[n%¾ï?&!œ¯ªiÇ?BÔÇEeä?DF]ÀD][?ï³¹6ܤË?~ö¾õUÐ?d¹zsÝG?c nnv?{Ƨ?±³!?xŒÕ?ïEx2Áž?…Aÿ"nh[?ÛÁ¬?{É:7³œa?•é§n±?|õćâ;?ïW­0ØÄ?…ˆÒæ±M?ƒŸ¬xÁ?tŸ~)¸u|?†uÉ5;?'SŽ@IÅAGN3FGL J2343.7+3437@ZÝþD5À:2Þ@'—GÀ:Iá`ÈWÀ;¼—•³[¿Öà"·Â@"†w}åß?üþ –
¿ïÿñ;äT?ïþ ûh%¿Ìi•Zo¸¿Ò·½áÍdøAGNbll?ïûÔ/JN?65¥V2m ?t_'Î&?g¢§?P?9Á_êJý?4¢UfÏ?ï\C	6ê?•¦5)¹@?rþ¹ê˜u?~j\H?p7Îâ÷h?'?ÃKSA?îúMä§a?R!fÖC†?VüJ7?kƶʍEŽ?˜0œR™¼?‰û/Ðl?¥¿d&?ƒÉlF<·?_1S€å?[¼y{=¤U?ƒò,(b)Ø?ƒ‰Ô6?ïý3åé1?2"Ztꪨ?=£.~ˆ?
ø1.]'?1'fvpQí?0ĄÀd:'?ïΦr+QÏ?rɨd"}q?Z‡1ç@?U=å3.®?r–N$Â?n{gT f?ït
ݏÏ?ƒ™óÖVÜV?uÌÓÍXù?ifäýyt¬?ˆÓe·!¼?'7[==Ð?ïè¯
7?Yïǁ<M?JJ£?;`ŠiQ%Ð?`¾s>£@B?W>ö†iÇAGN3FGL J2344.4+0549@W'?ïXÀJ¢‹ Z›À:5¾ aŸÀ;·"ÌÐþ‹?âqš¾ÿüò@"ÕÁ=!Ÿ@‹‹À"§¿ã3Ál;¿®f@q<â¿âÿñÊ)¦º¿ïôV©"ôAGNbcu?íÃ6že?©Aç«ö=‰?¦a¼´@?¤¤OõɋÉ?›lyw{'»?œ›ƒ!>!?Û­•Ê¤v?Îl@æ$6Á?Öú ðzý?ÉdTúiyR?̝אcÿž?½¿ô]p¯§?ççðס›?°œ»
3z?Ä0râSOf?ª¹¦ -Ö?¸fº¶T"]?¢'"ê #J?àLQqb?¼©÷lªð{?Ö¯1—áç?ÁšBÎ(?ÂLjžv¬?°÷î€gº?îƒ%_Ù/?¡–ÀzÄ»?Í®µdÅ4?˜þ$'ïK÷?'Í®åLò?"‰˜ÓG§?ä®r:žÑ+?Ȉ>¢Ö?ͦ6™f?üM-…IV?¿@	Ö©¬?°ŸWiÎnÆ?êLT5¦ó?©4 ¶1i?¿‰¨ÜhÝJ?¤Ÿ~í¾+l?¬'jñô 9?›häQà?èÌL¿ÿ½n?¯ñ£r•²?Äà‹~<?¯	u‰>äŠ?¯¹вI9?˜BށÛAGN3FGL J2345.2-1554@Plžà*w£ÀQ¿_ã•fÀ7>/GìÀ:ŽÞ¢¸&?ýdþ¿¹@ü½å©<¥?þ¹Rý(	^¿Ü±—¾ß5¿âFA¹¾J¿áº™ˆ@›¿æ¾ä½ëoAGNFSRQ?ïµi('Ð?ˆŸ«n'¶¥?7/0AKÿõ?85£Ðá?ì<YB«'?ˆŒ´8>P?ïlQâ˽?Œ9™…w¤?c¸öö¨Ó?tæ£;©?ƒ¶­ÚxñÖ?†{Òlœ?êZ±"¬?°'ɕÝ7Ù?¦p=¬h;C?›-ݔãTã?ÀùéÐé'ÿ?¬i'.°†?ïÞWCˆÀÙ?yåӇeµH?Tkš0¤n?(`<ì"dû?p¯µmJå?yÜ8·kæ}?ïß$×ê{ù?z/?ö÷€ó?.ÛJÝ8Ë?<!V
ÈÞ:?níwØJϝ?y·[ ?ïâ'1>³¼?k"£ù¦íé?MáÝdf?Nð-`5I?f"V‹‰Tã?eQv	h?êèûYۜ&?¬ŸŠç}'Ì?ªåwÈ ? bP3?»EioôôM?¦{¯§6¶?ïøHÆÃHj?Utp'°‡9?[9à5Rr?''DØÅ?MÇ0òs•?Të3<ßٖAGN3FGL J2346.7+0705@Xß֔ÍÀJ/&à>™™À9*NRsj[À;1dÂ!x ¿ðò㯽Gt@ì±Ííß?üu§ALü]?ï]cdÿ¿ææ»"!àG¿Á÷=ëTÚ¿ØKÈ·AGNbcu?ïìUM[ÊÎ?bÌIýžc?+ðԟSÒ?%7æ÷•£c?aúcÓý¢?bƒ}b~<Ø?ïœÙÿÓy?"ò¬A`?`ö|B³f?b]Ó ö?"Œ:ò€vÄ?'LÎ"r?îyzÀ:˜?˜óöŸh—l?ïêm?&Êð)w?¦ ðѾíõ?•ýgŠ­â_?íG°‹×Û?¤¶"ŸéÊ?&·Éü?+JG®:5?µ·lFoé?¤²!½Ï_Í?ï÷˜¯R­;?MžG·?+&2B?&ƆöªM?JØÝ«(ú?J²©w‹´˜?ïÞ+Š¥?j£³ãl­p?O{h°S¡¶?O2}·ø?jújꯌ?e€£úÒ?ï8҃^Þw?‡
ԑ´•@?'ÅëjEeß?vü^5ñy?sÆñøs?ƒPJM/£|?ï.öÌ$±?‡:óÝ­§?@€
Ãç?l¾Eä'u?š"$ÑÈ??‡1)_ù#"AGN3FGL J2347.0+5142@\8åÏxyÀ#Îã¿ØrÀ87¢ò(§À:éß÷KüX¿ñîéµ:ßÐ@u'Ý7©?ü…2ªÍ¿ØGÏQâJã¿Ù	žkÝÁ¿ÝëØM*øt¿×|ÞÀó®AAGNbll?ïÄ]Ofo¡?wBVønk
?8xµð8ú?4eŸE"?|IÌÒ¬	ß?vÐmßf?îÛ1¥ ?£"¢ió"?yZŒ…RC?€HþݧKÅ?žFsî^?¡0"*E¢?íÚT`e¬"? ‰t›MòÔ?šÂüxèÈ?ˆû#ùä›?ª
Xw?l?œ®qãŠ8?ïƑŸO;?Žñ"'ÙI?#41â
^v?+'âÚ0-?ÀÅ`$‹ƒ?Ž×¾8!"?ïïn!ñ—\?V1×\Ø|
?(™ßpÓÉÚ?!©iÇE?^€;[Ä?Tä÷ñ?ï~®9õÖB?˜͞3%T?f[g'RŒ?g›m¢?Š½—É·xæ?•¨3''ÔÏ?ï=1±¨Ùþ?‰ Ýû{°?m99•¡Š?|Høž¡G?FZ\‹ÔÜ?ƒ›·N°o?ﵤ¥ø]Û?q¬]õ•?ëµ/–™
?Ÿ$Q¹WÍ?'êÀn•Ã?qþ­›2dAGN3FGL J2347.9+5436@\ož²gÇÀ"•¿ðExÀ:…gÖ¨î¡À;³0¨LÀ
­óõ"@ÏTБÓR?û»ê^Øþ^?ïÇôЙWw¿Ø$ë"/š¿éqF_®¿°ÿçÆ5¡AGNbcu?ïN‰UÝ4Ø?"2¾¨£ ú?pW±¾8ÀR?qˆ£ÑÁ·?'èÚ™ô?'ð;Û±?î‡Õõ"?µ¹d3Ê÷y?zÚþ9f‰
?‰$hBž0
?¤'@åè—?³ýǝÏ8?íJ˜¾ìÿ?›äæ6ÃE? >«C\˜?Œ`P ÷ôÓ?«ÈÐg+Ë?"ÐÒ[{'ž?ï½='?‹_—q›å>ç÷–,·?Ùí"M‰î?€ª'ŒÙ?‹^ƒÙÊÔ?ï¼±ñu?z_/üJ%'?\.Øt¼£?`£Þ|"®N?z›Q=TP?w=Üw†À?ï|aüZ•3?ž/öz¶£—?hèþ_?r㴅,I?Šâû¨Ñq¬?›49u©¿?îÊeÑÞ?ŠWƹ®?'¡ÊŸÞȜ?4èL'ž?•{F€¢?2®!˶?ïô!pÏ1<?``ªžÔ^>'{—ì‰>¨ÔUºMð-?W»÷"oñG?`ýLfOAGN3FGL J2348.0-1630@Pe ÕúÀQøM@$³>À8@¨E.À;ýFèÞ?éûß+k‹@g
[@ŸmŠNοÖò"†ì)¿åG@ÿÞ*}рÕl¿æ—ÊšvAGNfsrq?ïûßu'd?8
ŒXßg?ktœb?¹ðÏe?:ý¹¿óD§?5–Œ³ø Î?ïž}DµwØ?‰Orî"äs?bu~1{?rÚÔF¬Í?ƒÃOIæU?'æí8=æ@?î¼…]T?'
QzŒ‡9?Œ Î`-ŽÅ?ð¶âƒÜ?š¨)
ò/?ŒŠ³æOi?ï_ƒYw{É?œòy
¬!?1uZDûú»?88Q}šk?"É¿bg9†?€òz
§?ïýï@Xú\?#~Îøà?3SgíÞA?
noMé‡û?&òU"‡?Ÿv‰~?ïà_õš1«?iúå¬Z??OMdT?Q&âÍ×5?gØvß:y­?cM{=Jÿ§?ïU¦u?…¯vC¶à"?€Çs"=é~?xÜ}Û'Lƒ?‰Ïa92?@að7Œ?ïܲäÕhc?e¨6}[¬?+Қ4Ä#;?$V•4CwN?pÇø©«Ô¿?e~ôAÖÜAGN3FGL J2348.4-5100@tTŒ_¿ƒ8ÀO¦¿Â"OÀ:AÖ²ÿœ-À;ôäq.A?æxނE®Ð@|+Nbc¢@r?³Ê¿â˜ .wüU¿àØÉEiþ¿è&•GœÄ¿ïÿYsÜ1AGNbcu?ïk—ƒñ$?ŽsàÎLÚ?–IM¾ß*?¼Âò(?fWÍЏ›?an×ÃZ¼?íKH•ðí"?®qF B7*?»È%o¼?›&'p"­?¬m'ñ‡?¦]ÝÃÏ?ì+"‰Ë"?¥éÒ5$K¥?µp¼öÀç?¡îƒ¾¬qº?¢e=xYΖ?=Oðù£?êm8\è¹<?¬A¿ìSJ·?·æH«IØ,?¤yY†E?´¯ôk¸ó?£ð""ÌEÖ?ïÈ¡:Þß?uõ÷'½`?v¼¨õÿŒm?tp¬Õ|nô?UœF·?LæÞ(¼M(?ï~8¦Jé?"i?Îeíß?ŠÛ–•ãi?†'{Ï$?''mœÕR?ˆoU£û'?îÖ)íº-?—džîšr ?¦$ášeüœ?"ÌZÛ ù?w‹Äó#?€l¥¸Ì¾?îeĄB´?ÊEo1!q? .Nߌ ?'Á4 Uó?'êѷƔõ?‡#üé²ýAGN3FGL J2350.4-3004@0ð›_lw"ÀS-ŸàÛxÀ9åÀ]RÁnÀ;ÂáåbÅÈ¿ìR@ƒl @ûÓ
ÔoX@¤ã@Ì¿çK˜³{Ô¿Ú·Éφ)i¿åÀ«°ÍÌ¿ÔÃUqÃß
AGNbll?ïù ÎèÂ?Bˆ;m,?"0{úkÉy?Ð…(r¥?Fð¥EÛ?AÆÄ7P?ï¦A—ÇSÞ?"w<ô&'?_­ÔôQ?bTÓÃîK2?'‹¤FBoì?=M]é6?ïC2bäâÔ?€ºÀƒðx?ƒ:Z¶±4Ç?sÑRƒ0§¸?‹ùŽR$?v%ªQ×Fü?ï'.œ£Ý?l:Â?%Õj,P	h?.K\Œ+Ë?‹]({Ôt§?WÎãf?ïü;@â?6‹ÞÊ÷Ï~?rpÅî?R]Â~h?8	t§€Ã?4Ik?ïã5k5œß?g×di¯Æ«?K_xQȏ?Mè\dͼŽ?eò¶uXUÜ?bmÃÿ~ç?ï¥ò»Ò\6?rØe€¼É?uhOI\G?hÃâæ¿:?wž™·
h›?fLíkÃ:"?ïë"Ãý#	?X@ŸÙTê›?6F9«>?-%~¸ZÔ?d.bÑóð?X¬ÑòAGN3FGL J2352.0+1752@Y⮁ˆ*ÜÀE_H *AóÀ9èéuyÿ À;½ŽK‡½Ï?ÕUÌËJ@Á@ —ºœH¡@ô_¸Í<¿ë
õ‰Y…'¿³íÁ±]'¿Ý:O®áK׿çóijMËAGNbll?ïâ'rýñ?kÙ=Lªf:?P<†ŽÅŽ?QîÖ{dà?eO·Ì€8Ú?f'ë¡1-?XšåŽ?ŸûÖTÔÑP?ƒ"R–ôx`?1xaï½? ±•Ì ü?›UºöM´?î¿u?…}?ÅÆÝÅN›?ŠxÚêï8?x=–;PÆ?šÔê¯_a?‹yHŽB‹?í­"Þ/i?ž5£ˆ­N‡?"¡x^,Ë?ˆ®ÿ¾Xï?«VõèÌs?˜æÓ´§¬?ïôÎ*ÖØ?~­­(gá?<d‰
*uÕ?fÝEÛùZà?N•
1Ÿ?sQÞ£¬3?ï¥.‡Ê0³?€m˜[?hQðÅEá?`ڜÅ{PU?€ŸáËü1-?|ÛZm*™?ïƒjóéÇ.?w̹)R?y%U½]Ve?f@ó4Êrä?''˜26??s¬vlv&t?ïM};¿ô¢?PúRE?€"u%âé?e[rèåè?Œ;á1ҙ?z%ö/Vå¬AGN3FGL J2353.3-4805@tw7À*ýÛÀP‹Ã¿ÝÑÀ:¯pÂ	û,À<
K³\¹?êgZ v±Ò@
ÕÇèa}É@x x™¿ì#ÞùÂq?ÝV'®àõñ¿Øhæ62õ~¿åÃ{GýxAGNbcu?ïؓ?•õ©?p˜)Dƒzç?\;õþ5+Ü?`¾l¢Ã¡n?iNŀíA2?hd°bĪn?éu…%hW?ÅP>Ö÷À?¹ˆCšh¹?»ywáÊ(?ºË";Üz?¶=ïmÄP=?í§v^½? t®|Ðl1? \f¿9­?"ê <,ùU?¥,‡³Ã/x?"6³Lµ"?ç'o…ì5?»êîmRá?É
O ž"?¹©r:ì `?±Øe3è5?§o˜@"å?ïݧ\ó‡?n3-n)6?TÝ舻ã?ZB­ò'"M?gêÆ#?gL"Á?íákã±s^?­X"8,?¡RºÇm?¢Vø"Ž³[? –†ý{9‰?šÒþRyÛ?îðªûàg?öÍßîÓã?''qø¯˜?ˆq½};¤x?šòdTöú?xE…$R~Ø?ìs~ö2ÕH?¢¨¢gqÉß?·cG6X(K? zzáÆÏ ?"g#íÉ?†õ'Ë%KÍAGN3FGL J2353.6-3037@,*"øÀS8[ÿÛÀ9öøŠ/À;½Ÿ_¬8À
ågù8'@=L|ÛGå@Bm€ac?îþ>Ôüò¿åŽ-'*'N¿á4òX«¿ë@–®Ù¿AGNbll?ïÓ¬>¦ž?wìŽì¾ðñ?h‰w"W‡?teÇ؍Ê?dÐÊ Š»?bwñFl«?ï"qÄm?‹¨¼Â֎I?d+‹³JÅI?eJQۏ3?…Øׄý#ƒ?ˆæIÀj?íjX,«žn?›B–v¦.æ?¨9絯š?•YAÑ
èõ?¡!lP$‡?5h´Í¼1?îÇêì¦?¡í÷»t?ISiâ,gŠ?bß+t"Ì?£)"ªÊÌö?¡¬U`"T?ïì¬Lh?_ïã¨?Sì]ð èò?Qy›Uf"ò?SÚ¢¡HÆ3?S4^Ãc#\?ïÜîFÞÐt?nݼÊÓMÇ?QÐʕ|i?Tg¯*i?j)SÞë݅?gª¾2`?m'S?'8Ûª|ƒ?šK"º?ŠåìEtï?åðp|%&?ƒT³KG'?ï¿%(rSÉ?|\'Ã¥?''ÓJ?-Cœl3%©?€3H˜$n?|'#(t£AGN3FGL J2353.7-3911@u'ÒÀa"ÀR>"ßöu=À:š—Ëc@AÀ<Õ,ß@¿î¹Ò@Ö@ƒÊ${à@?[?kд¿çxS¨'Ï¿ÛQ´}¡¿à'-Èä׿ïÿZãÁAGNbcu?îâc9¡?¢ÆO¾Ë?œ¶Dé>»?¡òº¨J?{õhחǁ?yqzF87Æ?ï.ã‹ç:?—¢¤¥ÔIö?x‰PVE»-?|CqJlI"?":d@K"?'ŒÙT¶è?é4íõ®˜?±®·¨?ÃVŒš"о?­mÔ ©ùÑ?¯Võ•yì"?™Ú'×'Õ?îÓ$…£öó?—7œiü ?u7ÓOΗy?'øÍWN? &½="‰Z?'»[{ÊÓX?ïp	–	tÑ?'}(hkm?‹z*…¾-?¾v"ÐÅ?qàG®Ù?pò'VÀ§?ïÀ)<~$b?ìyªÙºs?b°àlð£×?d[ºBàë?v'ñ`ÿ?x6ÔH†G}?ëé§}Õ:Q?¤¦Á\l—¢?¸ÝcO?¢ãåånü"?ŸTÒ»j¡?‹-š~,<?ïÇ?lÉÏ?qgQÙEê?JȦkÉۋ?HæmË	—Š?y%Ëp;?pÇÙ֝‰AGN3FGL J2354.1+4605@\+'ÿÀ/EšÀá@À9øÈHٍ¥À;Ñ*èáÖI?êÏ	\8ÿÀ@‡Á‰LÅV@Õ?qZ
¿ÞÆüE¥¿ä%~‹•¿îíi­÷'¿ïÿŒ"ÅÁ¸AGNfsrq?ë"»c?À4+§^åO?¾i?´ Ü?»î…ÞjÇ?£p;¦o!?¦Im) £©?ᜧؙ9?ȾÛP%åË?ÐySÑð?Áµìœ²?Țºøú?Á-ý/Qb"?èÂ,‰º˜1?²Lá"ìè?Ãw^)ð®?­Á{®Ër?²ÿß]Î?šÃRÓ÷l?ßKlTçãÔ?»u'1jÂ?ÙÚ9ŠeI?¾½Ê÷ñ¤Ú?»j-ÁëX?®Nӊb6?í¸J
·›?±ùˆO´!?©b踨·ö?ª€u…Ã?–0ìÔK"Ÿ?›
¡¤*?é©œºòk?ÁÙÓvñ4F?º"ˆÚð
?±Œd0í(?¸#ºA]W?·™˜›V'û?í
Yð¦
?ž6œŽ~Ú?°oÐÝe'Î?˜þEC?À–?1Nŏ?"–	?z?êlu'ºh'?¨ˆ'Ô;F¡?ÁºúiŠ˜?¤o
°ÐEg?¢L½/çGy?—"Ñû°œAGN3FGL J2355.5+8154@^7†6`å@3@à†7½À9撚Ϡ½À;ÊÛø¹º¡?Ú}'õ2@
áö#l@óðX•m¿épҌÄù¿çä{Óh¥ä¿èëh0"•¿éÃ剠ìäAGNfsrq?ïcUFÐÁE?ów<"´A?ƒLkèUDM?'"..?ƒÞBYƒŒb?….Š…i1?ìá"Æç?ºnÊ×ë	?««–·?©ëR¶®å?¦Òk:i;?²'0áîHÓ?í0î›^Ç?žRŠÁƒ{G?¡ŠÞWô®?äŸ¥—ì«?«f7óZá?"ÑSkÎ4u?è1†iQÓ?°Å½ÉU6?ÂÐù93ʪ?«|Ô.Csî?¸Ñܑ"?¥ç|þȬ?ïÉÁ‹êÉ&?{E¥ß '?nwæFÀ‹¥?olðò…"ß?gƍ¦šÖª?n–©:N˜?ï*VçÝ
Q?¡œøn3Û?‰Ññ…Ûúý?Šœ'WK°?‹˜T†PLÛ?™‡HÊyTb?îø¥³ƒO«?‡IXè?Ÿ'QâÐä?~Ìû'?'€è\p$?|}q-‰aþ?íîZ—Úä?"»ÅÍÏ?¥ÐzQ5ïÔ?‡µ¬€Ä9?–"ʈàõà?‡ÍòWDRAGN3FGL J2356.0+4037@[íÿ`Ï‰À5ÏÃøÀ9ávÐ@õ"À;ˆô›GõÚ»…Q¹@6û{6D?û+¿K"ä¿Õ¨ ,g´g¿ëvàêfÔ?ÑT'¹ó£ž¿×³δÀAGNbll?ïÆNzÙ²?†ˆ>6ù:?0!êÝc~?3éò˜?ˆ
]_?…ÜEõQc?ï"$d¼e?•èœýuc?j°'uYu?p•‰?]{Å?ˆJÔL€j?ŒiÒÔ9É?î:€âòÊ?–KSÎNÑ ?ŒÜ°
²Ô?{ßÚtóß?¥ ÅÊßh¯?"ˆÁÆc›?ïi6©§1?ï˜F
åÝ>ú=€=í
X?íùƒ—ÂU?'Ò›vq)?ëÀjÚ7›?ï×2€Ó"?r:ôݐÖ?,È}èô•?-—øÁR×r?s€{³{'I?qº|üŸŠ4?ïÕoÖ|£ë?q§ƒØ‹H¨?VGMmX_?Tú&ñâ($?oA…¨kY˜?k¿|]¦›?ïTƒyéóF?{G'"}!ª?~™pÿ÷?kä3ŽR^·?‹ÑÔï<*¬?u…éÁ«­­?ïá·YëP=?d[í¤y@>ò]áZ-xn>ôÝ;øû¸?n#ê/|!?cÿãkp9AGN3FGL J2357.3-0150@Wb‰ۂrÀNËä€G¸üÀ:h_¿ƒ8.À;çCHT,¨¿»ù´PBýD@³±"
‰F@üªß'!U¿©J·'Ú¼¿èÀ/³ªoˆ¿Ö¯ƒÓV @¿ãk<P,,AGNbll?ïè+/??a¥‰-?*SKl^G?&²ÕbŸ'?fUËL軔?`rË"î;?ïaþÏD?'aá"mˆÝ?púmńqÓ?y²y#6«?>	\|>?%I¾úw?îaN 2K=?ëzëa@?Žô'ï<¦?z"Œ»Èj(?¢-õA=?‰)T¡½¶w?íŠî‹cuñ? 'âøá'R?oàˆ[ý®v?mŠ»ÎÙ\Ÿ?²©‡bc? %m·ce?ïôEUʍ?M›ƒÝzY	?$ŠQ‰š?!eü¨Äo/?U8+$q¬?K¸¨…º–ç?ïÍ·×®cf?tÈAäX/?Zˆ9>â'?\ѯÝF?r'Ôÿ4J?ozºb'Hy?ïVozƒ¡,?zÏxü¨¡?ûj¡©?mk—Ì¥?Šfl[øî!?rz
ý?ïzÜ&~fZ?z;V½°àí?bSX¦º?O…À'—O¥?ŒÁჵy?xû@ë'·AGN3FGL J2357.4-1716@Q¯3+¦ÀR†–ÿöÅÅÀ:~I±ú¹À;¢I
5
(¿ðz)˜Õ¤@I—ö×7_?ü×›£¿åàQ*¸e¿Ø'-˜‹ôã¿Ø,ßÌT¿Õé†lý?˜AGNbll?ïî½6àE?]·kÙ?'Z›Tlzˆ?%÷F	o|?`"™9ÇÖÕ?\QZœ~ß?ï¢MÚuÏ1?…vЙ{Å?a&*Yð_B?b×Ã#q9?ƒ"þÃ!Þ?'c­v]»Û?ï§c0ÑÚ?"pŸ=0+Ô?ƒììVÍF?n|Ë«Û'¾?""s}W?Å¡KÄ?ï.æ¥f?‰}:¾Aï?#<'¾T?%èCòá?™ûð[/A/?‰s¿`Í?ïøùú¾ˆÍ?GÚÆÑ~*?wM¿"Ð?•$BHõ?IEñ÷?Fžõí62š?ï᫛q,Š?gÕ8˜ƒ2:?M4êQ9G?LÙÉ(‹6?g*-ˆsá?böj…ÒãÍ?ïF·?mzO#1Y?v¸Ýqש
?\8°)¹Æå?`
Éy«?fh°´»x"?ïÐ3V$]?c‰Ú‹†™R?+k¬#>?*ײû?wøH…²?c{OU¢yµAGN3FGL J2357.8-5310@tz WŽ\ÀO~`X/lÀ9*i;,ü¸À;{ªÙ\þ?ñÑv—áނ@g%%ÿ@¤Ï_ÏŠ¿Í@&€ó/¿èh®\Ê0e¿éÛ7¯Õ׿èõI¯»2àAGNfsrq?ï÷'%\?MUÏ"_u?D'ª"!?F‡˳±?:K¸I1"?7¡/Ø?ï‡i۔Ä?‰²&×zè¹?iuuÉÛ¬?ksàürju?‡È[4?]õ?…h¿"ÒuÞ?ípɋq/:?ŸXTÂßj?¦
Y§2«Æ?—¸¶"›?¢æ
žJĤ?'¤rcëNý?îjrìþèË? $Œ¦fèŠ?|ØbVˆ4.?vm-	9¼?¥½ÄèšC?ŸÝS5dÄ?ïù¼ÑÏbv?Cئˆ'J·?@wÿE8üó?@Úå!ÇZH?1)q¸R-I?('\ÓPV?ïÒ®¦F%S?pžÃG8ˆé?V†é<Óq?T­Æª"m³?q&9K_?j0x­¸¢Û?îx´kÏS\?—(å±³v?ŸÕ^Á¬?'çDhX½?'ØZ´&nÇ?†O¢2M
?ï"Àˆé£??b³ò?pGQBPÔ!?aç˒¥]—?'¬53Õ$?=ß͛)îAGN3FGL J2358.0-4552@tŽ§Ÿì™òÀQàÀ48À:
ÐW›ÈÀ;ñy¥Œ¿÷?ñ²ŠV@3¼ðáª@ïÕ`EK¿æîô´N¬¿ê8IÈuû¿äÎíöŠ'È¿µ"§?۞]AGNfsrq?ïûßZª+É?<<:j0‰?€P*!Yf?ò´r©}?=õ ûc"A?;k´Ð±ŒP?ï£Z§ã«®?Ši-qüg\?ct­cxê?{X$q¡?'LTã£PA?
Å.Ì0?"?ƒ,šv'?Õ6&zaŸ?jm¢õÊÄ?•¸Ñï¦5?€ù|¹Ïk?ïÚú[¥Œ?oÈ;›÷Ñ>ãƒ[ØKK>ðý)^ð?ry½àqU?oÀ7³¢.?ïýS3¹/?.jìYáµc?¿©
ÑäÁ?¤ÒŒð?2O˜ÇÂY?+Ô+'¼Â?ïãü 
]?jYýhž??Kp(1?Mà[˺?fÇ«X¾r?dYö}_¦(?ïž~q世?mEÈU& ?oß7G'Òa?ZA¹óQ'?€h•§.ö?inñ¿1?ïû4&«Ãñ?@¿Ü
1Ò>¿^¡¢¯>ÀuWô¿?CÕùyî0?@º7ÆâýAGN3FGL J2358.2-1022@Tæ@.Ä9ÀQDy î?À9ÿ`µL}‡À;ÛQk,žÄ?òYôèõ¢@é÷7"{¥@^ŀ'W³¿åãC;"ÿÒ¿ì7ä7ÍvÁ¿ï´xAk?ç€`'çαAGNfsrq?ïܐí¬	?qcԚZb?U|e‰Ð+…?VõÐÕ,±&?h°ß˜˜Èý?n2éÙBg?ýNR|?ˆ4£-"¢d?c°>6Ê?fœö·Fq?…3q$8!7?"m³ªú?ínübÁC?¡R×Ñ(J? ËòzcüÝ?•«KéOžÖ?¨DGfG¼ë?—×ڈQf³?ïTWB=	?›·àk5G?]2ü3D3Œ?Ÿ€…kÐ6?"¡Üš[q§?š D]v?ïím÷T_Ô?e•‹cg*Ì?CX纔6?H"êÜy?[w=6›?bù‹ëT'?ïÝC°"?l;Ú7Âk?Q£dyÌQ¬?S%—ß÷¹?iêå#å?e@a_2?î¿kzÍP«?"¦¬ÎE"?Žå5JûÖï?"½ÙÏE¡@?˜Ÿõÿ 1#?Öûoý?ïëF'
¯?wÃcYôÅ?>ÎîYº¡ä?aïüû‡V?aÛo©Ò?ruh%p	xAGN3FGL J2358.9+3926@\"aùðÀ6NÚ_\†êÀ:DýòÿfÀ;¯&2™°@À‰£µQ[@½v›<ÜÕ@ªóŸõST¿âDè´¬<¿àÖÙI»h¿ïp J3'
?ì–Î( ÞAGNfsrq?ïçTœ~?:?mɪÊ>¶?Q‡ ›|?W˜ÿóB:ä?_Ï%òIàQ?hsקjj?ïŠRõxñ?"›O.ïà+?mÈ@;.?€Ð±ç£Òª?…ù@ßsa"?DÅ_x¿?íì1€ok?›­OWKÙ?˜±%Дń?ŠÖË<½?¤æ©ýöؒ?–×›'øX?ïô	Øy†Ý?_zËPˆù>©EW'iÅY>ÕKScÑ÷?Wé&æ÷s?_zW@wú?ï÷ƒ¶³ø?SÖu7"¢¶?3¸[.Ò¯?:ôÿ"—û ?HúˆG?O°Å!®Y?ïڅ$Ë!?o35j­ä?TÉrÐÜÐ?SOGhWØÞ?k!Áz?hd}€Má?ï¬@<?‰¶]Œ²‡P?‡†~örŽ?zzTÛ%·i?'§=†¦Ý?"ë7_×oØ?ïþ·fÅB%?.@ÅW,)>ZNä#ü>m[ۅïí?$ˆÄKç-?.@Q4OÍ`AGN3FGL J2359.3-3038@)iÄupÅÀS"x $ÎÀ9½¹Ì?TÀ;¶°ê7.¿àêìX@
³¿e=W@,7žÞ¿ç1Ro°ßS¿ÞlŸÖI£7¿áœ¿^­½ñ¿Øê|"îËAGNbll?ïoNÙú)I?Ž!ž,È­P?Y•m?""£?R¿MÂZtí?|Íçò¤?
WMÂ÷#?·Þ?ˆTçˆ[?fBñ!®ç
?ix´¦¡#+?‡ê]CŒx?"õ¸+žø?íÖÖ
/¦-?š8£Ñ*?"ù·³ØV?;èÜ?¨•Ã'=Šå?•›m9Ìý?î7L«æ^?™ž-7Ì?Y¢÷þÙ¢?\Mm‰Ü¬?«¾‰2+<?™…ñwû.ø?ïӉË#?víµˆ·û?DÙßh?CF†ßbF?sŸùF0Ȗ?u`–£Z	¤?ïÜvciÿ?j"||‰[?RD‹Bm¸?Pð'
‰…?jg›(ê¡Ë?dˆÌ¿ü!×?ïHW:Wz?~›''èÖ?)%±tŸ?k‡òUu?ŒÁ­Æì?wDRqê6–?ï›"DÅÏ$?u"³®~:;?@¡Èb&Ø?3Øñk??ˆ-]{ô&µ?uJˆaPcƒAGN3FGL J2359.5-2052@Lù>À//˜ÀS'*ŸæºµÀ:Nè},{‰À;ë?Íui9ÀLEÓÉÁ@»ž6aeö@$6ßæ+¿èûAîs ð¿Þ",æ½å¿áZ˜U²ö¿¤­ca4ŠAGNbll?ïí®W§íÖ?V‰ÍA5°?'IþìôɅ?Zc?Á¿.?`ÝDJD`?U˂ž )%?š¤Â©?†5<ÆÜ},?`Ù8Þs^a?dÒ¼!×µ?'çË"ú2?'ÃCo—É?î°|(çÍ&?†5oDþ¯?‰OhË?p*gŒsÖ?fÓ2gg`?'NÖDOí?ï´Ýêxњ?{öxfFòŠ>ðögˆÏ£O>û§ö
©^Ç?'À
!7!p?{òXe¬ø?ï÷×6!?D/ÿÝø'?©žÆKX?
Ÿ
®æ.X?MMóï[=µ?CJö£p?ïâøXýÙE?i©JûʐÛ?L‰Ô]Ï@³?P_¾L1ò?eå1ÚWù¶?c=½¡á]?ïmÉ®N ?p»0w}û?zéC ù6C?]d›VÑQ¦?‡CìàÉ?iI¤"?$?ïó÷ˆz@?NÔc71»¡>Ë ×;ƒç>ÌhÔ"1#?XF¾"ÐT?N΃ŒˆAGN3FGL J0000.1+6545@]lh‡¨ÖM@9Aâù^üÀ9ðÇô À:æåèðð?óÇî@
©ÛÖU@I£@Œb$¿ÜTX
ÇÉ¿æRGÀ*tj¿í$[ÒK+¿ÕÕ¤l†fUNASNone?ħ:°ÄÈ?¾žÖ.ö7ª?ÑÐëÁjÕ?Ç£"3m?âàPžd@?Í	í\Â×3?à=ñZÔ??Ö$° ø%Ê?·i4¢Ïa?¹Ñ¡{?Ù©Ð!Úµ?Òìÿ}X›?àð)ôD?³­{Éô#?Ä<íKá?¥º;‰£?ÕË5Š%ˆ?²úç·v?ÖچÊÆ—?À¢§6‡æ?ɝlÍ]ÁQ?ÅÒ/¤Õ¯A?ÜVÂϝâ?Âd\o†dw?ÕXÔ@v?Èfò暆Ý?žoˆ4R©?»—uÆk?à«ùÝÉk¼?Ëî4¦zÔ?èIÖÿšø?Ñe­6
x?­nãüRò!?µÜ†o+˜?Ç|îäµÝÙ?Ë*6+Øma?çæ«Ìˆ??¬.:ö­
?¹¿i2¯»Ö? î:ñó—?Ŝ6¬åQ?§+™£	ñ?ã=üžæNm?·Oè†@?ăá'Ú?µÍ" †i?΄,[8ñõ?²i'ƒ0)FMIXED3FGL J0000.2-3738@u–'}keªÀR¼—žÖÜÀ:ÀঞdÚÀ<åS¬O?ÙÌd3ӎ@lþ.ϐ?ýÞ"?pq?Ã}¸X‡¼´?£ß!W tֿԐÞÎX¿ä½÷n®UáUNASNone?ïñtº3Y?YpK³¯ßÊ?6ä߄\¶?8ƒÛg{?W]SôCO?UÓÐHk¢e?ï?Ë5Y9h?"
öã¡¥'?v¢p÷ô¡³?|PجY†?']ýïÿŠ?ŽsK|*Gý?îÞXµp18?‰Æt‹E­"?‹|Ýü>R?zëG8Z-Ù?–vzU' Ú?ƒ*¶¯£tû?î=G‹?šjŒÀâ±?…ãÞQӉ	?ƒ¨DÅëQ?¢"8EZ–é?–îcQ\^¾?ïøMùªrÒ?\äu:ð?&:OÎC'?"ML^ª‰ê?I9˜6Â2?\ˆ´Ëus?ïÀø(xÍ¥?v	ƀ&?aß­ÞÚõ?]Ê0à&?v"3‹x:?q	â#?ïv‰hìJ
?wQSÊwpñ?~cd·Z×?m'(ú?ƒ+ó^Á`?ns}'ºŒ?ï"qžuBð?x1òJª¬?vØ=oªch?a=áë͂ý?~îóGõ´æ?s8	ۚËÁAGN3FGL J0001.6+3535@[êU!š"{À:0AÿŽÁÀ:iTz«—ÉÀ;Ý+€À…¿þ³LØç@ÒèDÍdw@ÍÞ?eñv¿í"O'…€¿×òp'@ƒö¿äSÿv¿Òw:/aÿUNASNone?ïáh™W»?gP,"Õ»[?T6þ´Cp›?[v>LB2?d{çtžXŠ?_/eËBRp?ïs{\d&h?'8šG¶ÅF?pfÿ6V&F?}¸úxÒ²¾?Ší©OêÚò?Œ,S߀Š?íxp±RÀ?›èɓÃ}?œäRôp_!?‰•óÞªò?ªËkæ½k?"p;‹ÔÞ?ïP½²¨‰?~D1]?&¶ùcf?0Õ:¼ŒáA?‹ÐøcPÓ?gl0aêÿ?ïé—Ý#T?&´'m	÷?D‰‹^7*?PõBýª?a^'wƲ?#˜´·ð+?ïÓö½"©#?rG¬B7æ?Võô¤ZOp?[^•žÏ™Ê?pG$	%>è?kžûT1?ïßMz?ƒe;H¡sŸ?‰2?>ð…Ø?zLñbå?ƒDyžÕØ?x9…^+‹?ïìPÛº¦Z?T©Û×éÍÅ>öÏ áY>õ*ìê+$X?c†?Ü!F?T"{éùAGN3FGL J0002.0-6722@sb9-Œ*ÀH‡ê=ö۔À:n»ØˆÂ²À;çŽ
^v?ÔQn:Mâ@¦€®ç	?ÿ#?B‹?·m¸\Nj¿àºj­{^¿Û"Ï2r¿ßÞqƒ±êUNASNone?ïóEm%%?Rí4Ù?'Ì%8f ?%`º¬ñž?V{ Ä·þª?PÈ9¡Øž?ïReRž?'-­&ˆ/?pkóæc™$?v'&ÚUf?'˜Pþ§
Á?Žæf ÒOÇ?ïօ»ÉÎ?jÉÍç?…ÂñdƒM­?qЍ{:?'ƒ¶™´»l?wã0çNS?î3ÒA'?—ðõ9í%w?u¥Ù»?r•ô6ÛI?ª€Ä¬/?–£b*Î?ïøÞlB¯Ž?AìwºH—‹?Ò|ýÀ)b?Rˆx¤bÙ?HËþè"ÿi?@VÉt¥©ø?ïÌ'G;?sԄÈsÖ?X»¶¼JŒ¬?Tҋk3[?sÊÑ?»;\?pÈqNDG?ïøø5ž?p>û|j#?xÌ4Áf³Ü?cÝvá.hÔ?€§‰…?etbô["?ï•ýk·Da?v&a®
Ìt?hkp"<?W\V°Ï_á?"eÈø}ð?s=L+D®ÞAGN3FGL J0003.4+3100@[½³R¨CÀ>¾¾zúr"À:v,­5À;à/Q&cA?ÑGˆ>Rv@
6v5ƒ@nB@p…¿æȼ¦º¿ãVîÆ
ª˜¿ìžr"Šq¿ë÷[DŽ—UNASNone?ìôŠfïŠ?À&³¢H-°?®†ôqô'x?¾ ë¦	r"?¢0e,tï?¤?'sâ?é8þGÝÓõ?Æ(¨šbE?¸Tõ#"Ý?¹…k³
{?¾1¸Ê6o~?¼~AÏXBa?ë"úíX?£'¡ìÛR?°³|ª·8?–'°'ð½?²´k=K÷?š$ÜÊþ?ä1P‰Òž•?ºïÂóÁ?Í9¾6Jه?¹×€©Î?Âÿ¢j¬$?®ÒBkU%±?îF4Qì0ë?ÃQŸåŽÌ?¤q˜°¾?Ã=lÍ]Á?Œ®Õ!!fA?'˜1k†+–?î	Ÿ«Mîm?²Q$Ù¨¥?›Šm ¥#&?£Î`p&}?¡ Î|†U?¦Îo©V?íýï]àÓ?"1 Fb5?¡Ê±53ìÖ?l~ÏP?œ¬±Ôláý?†©ôdÿ#°?í&´Ö?áx
Â?ªQ"sa"?"»¿tWg?¤¼KÐ%+?'ýšuűAGN3FGL J0003.5+5721@]Š	ÞÀ¥yÞonÀ9ó"#]ÓÀ;…KQ7*9?ã,%2£v@€ÎۚÅê@vç?¿³Š?ïóšÇ'X¿ääëÿd.¿åÌ3Õoˆ¤¿â¾j}£ÊUNASNone?ìÑÑS'?´ŒÅ3›ûÙ?"ŠžÊéæ?•…@êêC?´U1ñÐÎu?²ÑGMúèG?ÝK˶Þ_-?Ô(ÎFZ¾y?¿?•$?ÀbºèÒE?ÙT"~ŸÆ?Ð$
o™á?ëÍÑzd'Ð?¥.îâæ€?§í"ìþ	u?•榶ºF?µš±´§îÅ? QE¶3&?ݗæ'+ø=?¼_€²Ü¥w?ʏ'i•3È?¾ßž
þµ?Õ …¹	mß?½–fÎ?ïfJje?¡%¬©?¼?zÏ3MÇ?€óõÒ÷ֈ?—?rlë!?I©çüpW?æîk#u·"?ÑZn&ŠiŒ?µ#X©@?¸ó,Éq*?É´§öì?ɛîúZ_Ù?î{%ߧ^Ã?''yýƒ
?"í?\W?'·Ó6ål›?œ®µœY'?ŒÄ—³¶1r?苏«·±æ?®D¨FGÇ?¹ëÔÂî^?¤úÖB¾×Ç?ÀÛÖïª69?¦óøŸ-sAGN3FGL J0004.2+6757@] •þÚf@ùÛ"Ðå`À9&ÀÀ:×t4…BÊ?õÓ.»ª:§@fyHì-@ù…±;!¿—è–¤>/³¿éì¶¥K²¿ålÙ¿pæ¿ëN§.œdiUNASNone?Ä"º
eM?½ô¬²"®?ÞCŽ®Ê?Ì:*5€?׫PoC?Êf'¤:ü?ÁÃ^v?ÄÕRÐ?Ú•¥Ä?Ç0>rg·°?ÝgÚ ?ȘŸhæsg?Ô798l`?²µPK2]"?Ö¡Á¶™.»?²×ݸÚ?Õ'
ž¤?´#ÉÂX	?»,¦Ú¨`:?§OÄ#àù¸?ݠҟù ?Áw®ôZì?۔ªPîQ?½ª\Ü
=­?̤!^ ?çÿÅ¿ß¡?Úwü&'Í?Ê€u—m?×5ó
½âé?É_sê?ÓW.94$?Ѕ°Õ0¯±?×nÚA9ä?ƾÕs•o?Õ9÷…æ'ø?Æ,‹6²ø?â˜ry¯?±æÑ­µ™û?Ïx[é=?¬Þè@6J?Æ'kšˆ?¨Ëwä¦1?ÆMËB'¨'?©—Ò§Ô±"?á åh
g?µŽÜ!¢"É?љ"çê?°"¶¢0D€MIXED3FGL J0004.2+0843@Yæ^NÜÀJ.ý›¡²À:‰Ù\'HCÀ;Ü=TeF¿ÎJ¬)FÔ@ƒš›ø@gN``=¿è)þ_R16¿Þ'&ˆªÞæ?CC瘿ëÜC·(ºxUNASNone?ïÀΙրU?'Û<±&V?k\On¢©ô?pÜ$‰oP€?qê‹D±PÁ?zßóš¿Òõ?ï{ቯ?¤µpfyÅ?{·ïQÓN?>΅Ö6?˜ÐË|_?¡ÍZ'Ò?ëásë_4?¦½r•2|‹?±˜Qû Iâ? ¡ôŽ¶%f?®¸O\ŽÀ?tmÍÿJû?î'!Y'I×? g@cº"?i'†YÞ\.?s•ùBHêH?¥[rßaJ?Ÿ~?êßY?ïËæ[FÖ1?¡3ô•'íÁ?eaÈ»{ܼ?{x!?n·ÛÎóB­?ž¢…oxÛI?ï´À€ÿÍ?"êûnÈK
?eSêþÞP?f

?›?zö$"3O?3/üø±©?íZ›÷³"?¡†v†'?«ηÿ"o?›/Uƒ¿?ž‡Ù¢\Ý?'·è(щ?廬þ¢‡Õ?v-ß%-Ñ?_+Ø|' ²?V'Å¿4,?'yÅ@IòÁ?s—BKÞá†AGN3FGL J0006.2+0135@Y¡ß¹8›ÀM¥ÿ¼ä!}À:gÇÐ䉂À;åÅÌ'‹_¿üuB¿Ã$@§¡ïÿW@~Å ]®¿ãÙCӔg¿â>$A‡¿ä§³ª*Ð'¿ÙJµïˆUNASNone?ïè­ãs`?a7J$×qâ?6ñ9æY?4%€".?d#á+Š?`"S
ó0?ŽŒþ´?‡~Ò²®­A?b;5fs6?s§û«O?'Ï	Ì?s^'Ρ~?î"þ~íé?åV+ƒ…?}Ù3][˜?|Ó§o¹?V÷|†‹?"ÛØÕÚí–?ï§-E½?|ì}‰q?Éä5P™?H;°Ùó?†
‹©~Ú?|ÕæÑÁ5?ïôx¿É?Q¯È6enÑ?)8Ý?bP?#~"j€?TÕò_‹ZW?P³3œ½?ï᜻­Q?iœa«Õ$?M²¦Æ«?OÑhE-³ê?f÷SœQà>?cœÃ=ى²?ïm`ÌڟÚ?sŽç
· ?€¨@.xù?j{Š…?Œ?"£$˜÷ÄX?f­DPüÅ?ïðÔ¯ÖX"?QŸ  AÎ>é)çd0Ùð>è¯ç{Sø?^$LHT˜ä?Q"Xþš|AGN3FGL J0006.6+4618@\ºÚQÎÀ/»µà÷üüÀ:4š"U•^À;µ/ê©¿²¡¿ï‹ìò@èé­@VŒ?"鬿ëªü ¶*¿çùÖŒ
˜¿æ÷/Jàè?ªƒÉ<Ž@UNASNone?ïòđ¦?V_6©¡?H§>U'?LÔCXô—?LF}XÓå?JÈ5?Ëh?ï]$ÜtÏ?–uÂÖ¨
"?s¨	Jr
?ƒ¯!>‰À˜?ŽâÀðn¿0?Ò¯4Âq®?îƒ\T›?Ž{ÐGõp?'šñÞT4?}2"X™Å÷?ž~ã'/®i?†wyt>µ?ï9zžgð»?QvÏy¬?E_ژ
à?Sf'¨Jú?˜%­e]º·?m»¦Q?ïö¡nǀT?x@C'Ï'G?5n´r?Jèö>§c?JÃ<ˆ _?wúÃu0á?ïÌàå]'?vÉé{3º?['óÕp4?]6¹ì$ ?s3'ŠKêÚ?qu'jYœË?ïoðFN™?tUêVñ4}?ç«Ž*?iŠ$inÉ?"±ÐsÕ¢¥?jdnØèqi?ïÞòt"¿Ë?d ¹Ùü[?-ÛZ¶©?1úÿ÷P?o<mùh›O?dç Ù˜ÿAGN3FGL J0007.4+1742@[<ÝÖàLÀEô™÷LÀ:kå˜u­+À;âƉ¼­¿ÌûÛqïö6@ºS«x¿.@~á`'¡°¿ãøÏE^?¿äl¡¡¥¿åx¨åx&¿Ý@—UUNASNone?ïÇ7c2n+?w¯,ó
X?Gyv"ÒÄ?GÓc÷³'?yu·4p?v'S•
>?ïlÉøj?`jÁv?kÔÙ։…Ä?v¬÷y±O?Ø‡½rB?ŠZxb
Ø?îHð^Í?ä?'Ýу ?"ŽÃf<Q?!o½X_Å?¡)˜@-`™?‰âå[ò–¡?îë•)>à?üëؾŽ?`ý¬Üt%?^§/¯E'|? 6ҝBÜÏ?
(=©^?ïïãà¢J?[d–Ž2?0Š¥1pvÑ?-æ`‰™ÚW?\–Æ?YsÒñ»)ó?ïÓÀ=ꓪ?p•u.•"Ÿ?T¥øÀÐ#?R[6ž(õÅ?pöbùnžH?k2ÄPŽý ?ï`¶Âìœ?v>L³
?—g&ìh?j^|6È?†c+-F·?koa'ßHÍ?ïËʈœ=°?gÿ=ÐT?Gd…qëp×?9iG}³œ?w.+kßT?fŒ¦3^eâAGN3FGL J0007.9+4006@\~‰ô
(xÀ6Ø@žUÁÀ:[	Pá™ãÀ;Ï®KØE§¿•Yl‹w¥@Xö§¼@4p yr2¿ÎBœƒj€¿é$íú]Ãn¿Ýn‹ðò›¿âÝ«{]2OUNASNone?ïÏܦ?0zGmu?Eçm
Âk?Pœ£ÕSÏK?uƒ$({Žµ?€©ðn6?ï% ¸ò¥O?›ä>È,?x£…š+¸?z9£à#|–?•#"Ðž??˜õúç"¿?îgû$àn?'&t—J˜?'ŽÜ-þZ?rAdv? 8ß©ûõ?ˆçQ+Ui?îe<VÒ)?" 8̗v?lßw1U[©?hl³àJ¦?§ÞC,O"=?"¦[uòu?ïò¼ÞJ×?h¹¤`ÐÛ?.rÛn»>¼?GRݸÙ2è?X*õu°*?d}WÂ}IG?ﺘr°ª5?~XLKã?aäµî¯5»?]"P—‡¤?yÁkŽ§Ô?z§ÔŒ"¢?ïbѝ…Ñ*?y%®hÈ;O?1*ýª?pó}‰Z?†.glV݋?o8ÚFÇâp?ï¨RKž±S?qFÈùÇïP?_?Uã?Ji™
‰÷š?ù[ Ç&?o¢dm¹©AGN3FGL J0008.3+1456@ZënÀY!ÀGT<}^ÐpÀ:W´üÀ;Ï÷1$e:?ÜÉr¢éO@PM7–DP@(	_Ð=¿ß¬Ýƒ€Ü¿áqK²0n¿åT†e<ù8¿å£Y
ÄeUNASNone?ïZQ¢+…â?'~'P­ ?YÀ-¯?†g‡eÉå:?ˆ×H×ê?ˆQ"I*Î?í>‰)×6U?´EÅ9¹ã?™¡nlF? RcÒ?¯Fç®Æ°?­ãU¡È?ìý¹à£f? d¼l'R?¢Œ¼®Ÿú­?'l$°h:?­—±¦Åjó?"ºõ<‹)G?è‡&1dsi?®ôAäYŽð?µß¡ÜKT?¤vü:ítŠ?Ãa÷i·p?©
1Ï^a/?ï׌mOþ_?{¿»ì{¦?U¼WJpçÌ?_ĤZõã?m•fâíµx?x䤘p?ï:°ÚAÄ4?›´Ñ³?̓‡-¹%?‡2
‰ÞË?¶ƒÎðØ4?"`Çå7D?îý!œe"r?…™bPÒâX?Œ¥·ã_?{bŸ\C?'	™5?y]ŠûÁ3ì?í²z"µ?"(#©‹%Ï?¡YQì6™?…]Aa¶?£üe¹?‹5œ¬¥cAGN3FGL J0010.5-1425@UbMÒñªÀR‡&k¤"ÉÀ:"¢ïƒ°úÀ;þŸ¹™ê?ðÃ?ó`	€@#v4åç@w_»ýG?ï÷"ÁÄO¿åä6j—šÞ¿èŠ(‰¥Ên¿ïÿ†S>ÁUNASNone?íî\Ò=úâ?²‹ƒnö2?«mn¸,rH?±hnJjÅ6?†³Ï~H?‡mJB?éï™:hd?ÐP£930?¶ž~قpf?·ŠÊâ¦x±?¹ä¸¦Ð
õ?µ±,Ÿz—?æ`²67c?µâ F˜?Ëé]sšù¸?±ÀFÑ"²?·²?…Îvö?¡&–¬O4ä?âÄÿKؤ$?¿pc)ðê8?ÐgöHòL?ºÉ
 `-ù?Ä>¹V×?¶"ŽœDØ?îµkl'?§ÛÓ@}uV? Ñmæt´?¥"_h³W7?~òZúÇ6Ù?€k@Fb}?í%é\‹­Y?´w¬u`?¨'ïÆ•Ö?«Ò¶¹ÃŽ=?¥yzu"?¡–†¥Ý0?êKgT?©row?À¥ðZ»?¥±0:å—?¨±ÏžÍÛÍ?–SÛÞÞSO?ë4»sâ?ªº¡ÎÊ1?ºít'o?£üÍ!"«?¦Úö%h?Ÿ–˜ÍÄÐAGN3FGL J0014.3-0455@XåÄØì–ÀP†"&þrÀ9ÁÉ@PR(À;råB˜I?¯ZP ²Z¹@÷ä÷»ãÆ@MŽÆ,¿ãVaHæ¿êx.ÉRU¿àhà1®y¿ça6+¾¨OUNASNone?ïé%E^ÙÕ?b¦
è˜Q½?0ÿ¯ÁÁjý?+oüސ:Ò?dºÄg­?aèî{Q9Ã?ïp'B©·Ž?ŽÒ£rز?mÁ¡ŸØx?wŠÏ hu?Œoþ3è‰?ˆ…03­	A?îDq›é¢?"m&@}ëá?ŽÃ:³ã¥?x‡ò]U?¤*–¸…ñ?–Äϓ¬?ì még-?£Ã°ÍËvø?tz×Õ?lêZV)®­?½¼iç^?£^VBD¾?ïùƒˆ¤î{?HÆt}ß3—? aeôµ'A?A¤¸oÛ?Eك'ˆùB?@Vs"v=û?ïЗŽ–J?r–€ÞUl?XX­;p7?W5"¨¥?qž
I"3‹?ml¿Î?ïl¶¡/?v}ê‹Ÿ?yßï*y?fêV\/?‡â`:…ëp?q~=^	"Œ?îéÖîcËW?ƒ—ê+P¤?kÓ´•¨?T¢ª‰ˆÙÉ?ŸJ¿_ߋ,?'Þ\§UÛÞAGN3FGL J0016.5+1713@[ÉÐúX÷ÀFlÖÓõ¶À:n‹†±_‰À;ß-(W7?ê	UŽIPÎ@¾¨×Ð@D`Þ<¿âŒ]`â¿ä¸—G¿íDŽ $ô½¿Õ°æØÍ®UNASNone?ï"ÚV†s?™$Œ c—'?z~Çù®Î#?ŠŠµ6iZ?Š†.fF?Ž¡¹g"ƒ?ï:;ô‡k?œ9‹?x`Æ?sé"[vu·?'vS@W?"¾;ÃQG?–õ¨õ=j?íX€Ã›?¡&OV÷ªé? ç»Ì°ƒ|?'€ w¤ê??©7ö/q?šüÛÕ ¨N?í|^è:2ù?§±ßË'?•GºÖ_…'?™mËЋ?­–4À¡?¢ÏY¶Su?ï\ 	ÓÆð?«×L®m?}{¶t誏?˜1úŠ08?Š"`À»?¢C="сê?ïÅ
úõ?€As'Áä´?]"/»Öš?i© ŒÏÊ?uÛ»•&t1?w;e5S¾Ø?îݦ¨ É?'ˆy×IŒî?°…»¸Ÿ¼?†ÚºÞÿ"Œ?"¯jÝ:?ˆ/'€v¨–?ïv»R8?†K$ÖT?|3¾éø;A?x`i—1V-?"7ZöÍ҈?}|ÒÄt—äAGN3FGL J0017.1+1445@[«úëÄ	ÀG¥‰›õ"lÀ:"ùdoÀ;Ô_rV_?ĬÌɔ*'@³0ÅŜ'?þ àÀt¤Ã?ïûÛµÔ¹¿Ú›j"ÍNA¿èÇú¼#\?¦´+]UNASNone?ï¿jXäG¾?}´7{O?Vïµ[tK~?Y&œŒ"(¼?zŽæRâx?{ËÐá!›?ïc÷ñtL?–QwµÑÛ?læ>`'zö?{x½-€í?È«±ÈZ9?'Šÿ‡íÇ?íîÎÛ"ƒ–?•I9ÚÂ-â?™‰M€˜??‡B6)‰q?¤NkŠ÷ò?Žš|©¯øg?ín)J?¬"Ø2n?|Ml™­!ù?‡òд¼I?²Éܵ%¥Ò?«À¼hé‡õ?ïèíiÐS??eÏ|áS¤??¾\y"E?@ŠøFñ&®?cʘ×]8?cäŠEv&W?ïÑ<BGð|?u˜/‹"À0?UÚMTKМ?ZwCؘŠ?qëKh¸>?q;¦6o"›?îý'è…Á?ˆ5œ³Ä,?‹†óh†Àé?xŠoWHÅ?'Œ)AãgR?ƒj}2–çI?ïŠü®or1?"Ç yBó+?W²"ÔϦJ?[¥¶-?ŠJ8*Ò?ƒ'ô2YAGN3FGL J0020.9+0323@[ªà"ÀMLæ¯ÌáÆÀ:Š£×
=qÀ;º™?׆d?Û±±=¥'@ù˳G@?ú=	þ±vZ¿ïöjÌ;?ïüÃ'I¿É§Õ"Öó¿Þx&ŸH|"UNASNone?ïüêg΁"?0V•X?@5Uu–?(z@ö_Ø?2\´"-Ó?,J¡£œQ¦?ïq›^s[u?Ý
.3;Ž?n–]
	Á?w[JÓ?‹ó',™®@?‰2áȕ,8?ï1ß[Î:"?'eOqΕ¢?'+W`tl?qDâ'ƾƒ?®hÿ5\?}&EРí"?ï>rûä×?'"Ùy?x{Òé?w'na†?'Ü•è?ëoЍ?ïýÒ85ô?#à–À-õ¯?Iy€a?	ñ‹•½GM?)»#?Šþ›? lÇH£ùO?ïÒ%­?rÕ¶FÞï?WùÌ,|&?X¹"Oî?pòúh¦Y‰?m1þ=?ï–Äkeã?tµ¹ÒÇ?u­l~;@ß?h)½xyîî?~ð]â:?mN'»½Ô4?ïÀ‡ 4Í?pù#WGƒ?k7ŒÖ¥,?ZÿákÒ s?r áŠëŸ*?k|ä»ÏÒAGN3FGL J0022.7+4651@]uõ׈²À/xpCßÀ:4Õh-À;ºÊá:B¿úŸ/¸ªUÿ@
"€`7£/@F/ßÁœ¿ë"Øz³ƒ¿â"ß½Y+.¿çŃþZl¿ïÿî¼zˆ÷UNASNone?ìX!-†B?À|—«,ê?£òª¸íö?¨?†»Ç?³±ýA|t?»f.ï<õe?î@ÕIëRì?³KKº¨-?ZÖl1!?Ÿ¬!z†Ö_?£«ýõ8Ñ®?¬&"e_=C?è7ë7W@j?±æt¬üØ?»Ê#$G]?¢¢ï™*ˆë?Á;AŽYŽV?¯6ÌúÙ ?í³ŸÏ5)O?¥-|™fj"?‡£•W%è?díMGqß?®þZ(3ˆ•?¢°fDj?ë'ö¢ê?Æ«÷!+–(?¤—$XÖ¯?¬|ÙäE6?¼t¸Â1pï?Ã5Tl'¤?ïŒdtÉ«…?"­‰J­+?q'V¶éO?'©_õà?"S7dº!¡?;>ë.Sÿ?ësLï$™?¦Š_ª_ˆ?²‡PŸËO?œùŸŸµ?ý?±ÞGé5©©? ˜²â˜ß?ï"áÆP~??Æa'ÖÛ?LjÏÒê?WyöÌ/¯ú?×ÃG~I?HåâžvrAGN3FGL J0026.2-4812@s¥í»YÝÂÀQ°J¶¸À:[7 '½´À<
Õ«˜ ¿Ù-jôb	'@ŠBÅøG@ù1~'¿Ú/õ¾*¿ÝOõd}¿äï7+ª¿á{Æ!ü™UNASNone?ïõÁ<\?MáŠíz&»?9V+VÍÝ?: ¸¹ ¥ ?LP'IÞ²'?E.Æüô>?ïŒÉ}±F?ŠFÖÔ²?fʽüŠ‹?t¨Z£¨?‡Qƒ×ñ?"P"¶î¤?î¬cgGP»?ŒwžÜŸ^È?'söÚ­Ú?«zZÄ^?—ÿœ<h}?`:0])ú?ï:CW˜˜?‹}ì™™y?Z䡑H?W½¿×È[?—-{t{¹?Š¥G{(e0?ïú­Šã?R®Â®åS?)éúv>ì*?I^#2Ûî9?=¢Æ©ž$¾?<¬î,³}l?ïÜ×î'Ä?lZ'ATo?Q}÷•¸åj?PöhåÆ?k4, %)§?f~Ïfv«Õ?ïr7 *Wl?w6œTK*?aCº³{]?qýß6'X??'Ô+@kš?eµ$IÁV*?ïܬ˜Ê¢?eÍx?–Î?=ùõhðâ?07¾QñÑ?o²Htˆr?dõ´üç;ÍAGN3FGL J0031.2-2320@Qà% …²ÀUŸS À:§H>]À<
àO`d?âêñ3ša@;7äs@ç`Kð?¬ûÕ¿ÜSÜÉ͜‰¿â—=x¨Õ™¿ïøô
Œ
HUNASNone?î™Q"Eä*? !%%[? þ;¼—?žˆ~\êü?…³aøµ·F?'E0GÖ¦?à"ѽﱡ?ÑPÍß¿?җø7gRþ?ʚ‡"HÁ?È|șr"'?Á3q'Œa?èðçÞB?­Ü"@ñ
?ÁïDþ¯w?§ã"[äz?´š7)½? ëÎÔÀ?Þôc³â?Á÷ñ­p«?Õ/"z×W?Â=n0ÆW¤?Ƀ
ïŠoŽ?·,I[©ú?îû'çòå?—•ƒ-ž(2?—cÎiVœ?"°×´îoñ?'t3Vm?}'[ª?æÌg>Ózf?Éјr–å#?Ç],ï»~?ÂÙõ‡à?ºâlå92Ú?³Î9*
n?ê­Ý†-?¨Å"ëA¤?½0'DÏV?£_¾ø?ªÁPÝ?™"utIž?é=S™@iŽ?°MOðipB?ÁTê¨æj?ªk (k?³käüæ½?£ÐsJzw•AGN3FGL J0031.6+0938@\¶ñ€
|ÀJtîõÀ:.´iÿxÀ;»²åšùì¿ßçQu
›@
ãtÈG@Aë>":¿á‰Ñ¤fÀî¿ì€|Má¿â
N×æ¿ÄÃ9TyBÑUNASNone?ïÏÙÆ|É?x¸×'tmG?1!Ñ_·é×?;/ÿm›'?wlv~~r?x\"ôô™§?ïKó™mû?¢°Mœ2T?sࢸîEÞ?‰SÚNé¾?'‰s¥¡â)?š|ÜÁÙÌ?ìó>Ú‡?ž!Yµá ?™1Õ«#;?†ƒá­vÉ ?²"é›(?™éø¼Ì*?ívå'j/Ò?¥iÎgí?[·©"Ñrh?eþ»Fyv?³ÙøºNf?¥JÝæ"ÿÌ?ïéRŠÍŠ?s*±îEá•?!!ZÚôã?%î& @'?e›_}ý#‡?rÏôÓ[Ç#?ïɹñ"S?"mï¸ÝF5?]%ëc6©?p«œ•â?sٌ0¡ô·?{!Jû–VÌ?îÞӝÔð:?‰(yiúúÅ?†ëg19?zäÒf
"7?˜¯üŠê$-?ƒ~tqæP?ïˆæ`N
?}€ò×ïå?B¹©	°Ó?@e{žm?Œšà\Þ?} -HÂÏcAGN3FGL J0032.3-5522@sI輜$ÀNÆ6!úü‹À98ҙ•gÜÀ;ÆNóƒû?ÔVÆÚ´/â@ñ=ÐE'@2YÀe¶=¿×†Pn¿åÀ_±krj¿åþ.æ꨿ãú¹˜xÃqUNASNone?ïüR˜ËŠÐ?FD&¿§¥? _™Rº?'X¯L_%Œ?5j‹óö/š?A¤ï¢]"?ï©=ÀCÁ:?‡O®77.'?a‡FAk!ç?sñ3»A«?N¾\M/?>á-×?ïo¡}Ç?‡‹8@f·?ŠŸÚÁÑó?~¤ºU! ?''2,Ÿ†ž?»Jv¢Dø?ïö°óQj?YËø̏ý>íÿ¸R" ?‡ó"Ê"?Rbç‹ä«?Y³Ò!ã•?ïäíŸ$-?©A«[8
?MoW
yÒ?Š*UnhŽ?c¶›O¬±"?£¼fv9j?ïã;×¥ "?iÐy6Æ
]?L¼ùîÐêl?Oýv2|ß ?e"é©JëL?c'lòÀ©?ïƒm+bÀ{?|ÅíŸÕÎ?}@µ"qO?rÓöü¼ú«?€"ZŠÀƒØ?tì4m¥(?ïþÆ÷öœ)?1$'Xk>؝â´\>ãÔH%‡?"ύš>ìÔ?0û)ÆAGN3FGL J0032.5+3912@]¼ãÿï9À7ƒIàâiÀ:L‡È¶½—À;ظÙÐÁN¿ØûÒ4{îÊ@|ž©£ÒØ@'â?û˜'¿í–W£]›¿ä®Ús~|Þ¿à¹ýЃn=¿àFÊڐŸUNASNone?ïåeÚû8Æ?gN)nG?9ƒpkðz?57G2º?gi·Ìæ@?fÿ'ä÷û?ï÷ÿ*˜?¤ªqŒ—úô?€Ù ÿê0?ŽD§¡÷?—z"ƒ¥Èn?Ÿ@÷«A—?큋JBæ§?™ðq"-N6?–½O!ƒÂ?€«Ž,ÒÛ?¬ˆ£È´žµ?•›•e;ö?è<%0?"XÓé™?k0Ž¦ÁZ?i^2o?¤'("§J?'s‡
ÿ=?ïõÄr‹7×?O%Pào ?'Ærƒ;O?#wø§m?Q~L/Z?ú?LGQÙ\t?ﲿš'3?‰r¯la ?f óˆî0?u	êõÌ´?{¤ö¶?!Ë;YÄ?ï'DÊVÈ0?€ÀçlÝb??''{O›
•?jb$à/ç?'ΩåG®?zÈ÷e´³#?ï¹	0?n{"þ®·?TzvSxó?D
{Wwi?~!Úh¿M³?la˜3X–AGN3FGL J0048.1-6343@rø‡~äâmÀJ²D¿L±‰À:G./¾3­À;þö ƒ-G?óeø¸
"'@šUéŸì@Þ Z¾h?ïú$ƒíàÄ¿Ü®x¨‹ò¿âÓ2þ§L¿ê‡'éô'UNASNone?êE¾êGBE?Á6+jçÕg?Äýô"×?À¬Qƒ³Ý?"H3!Iä–?521˜Ý?é$wK;Ï?…~¸tB?¸Ž$×ùò7?·Us•?¾N ΛrÑ?µ€"͔,?âuü*!U?¼
'zn04?Ôù¤L·#ÿ?¹Ë‰§oV`?¸iy…?¢
8²ó ?äL¼îL=4?¼(ªI?Îå:•/Û?µá.{åêÛ?¿Ï£c>`/?²V§'C˜?í…dˆñ?µ95`ú?´ˆBW"y?´Befcü?""QƒoÕ?‰m¼ü?ìÐí€
°?²þ'Âá"8?©á5PÏ
_?¨W"™2=*?©ò¯hœ?£×‡/lje?ê	Òï&#?¯Žµ'0Ü?â¸òOh?«‡ÇÈÌ¥?¥[F(¬'2?'én–3?ëFšø(?¨pz]á?½ˆÄ4Lã³?¡Ù¦ªó4ö? "ÖD?˜N6Ã]WAGN3FGL J0049.0+4224@^'Ó"wÀ4tÙù9üÀ:mã؂µÀ;Ò?R%f¿Þo£78a¬@""^žñÈ?ü>ñŸêìs?ãˆ)ºc"£¿çÏÅ^)½$¿Ë÷W<쉿ÒIûÒ·ëUNASNone?ï³ù4gnW?‹ål1Õ°¹?,³Ù‹.¨ä?2.Cí^?'Žã…ex?‹Ài¶(ÐÂ?ïK9æ;ïÖ?¡e6²æéü?tXu°ôR?ˆÙ!±åòŒ?''¥Äò¤'?žÓ}4?î!ƒX?•ôÎAä?‹öGÛ»ñì?zp!,ÍÌÓ?¦é|.Dy?"Ý!*]{Ð?îŽOCFÒ?—tK)¿¯?G^·,x|Ð?Ol»
ّâ?¦½•aƒž?—V¡Ä­»Ý?ïÎÏuÀîÀ? ºüŽ"?1ðM¬àÔs?iõ…HG?wy@[®];? 9ôA«¨?ïÉHƒŽ?w‰ûDn?[뙭ñÙa?XÙ>	üß3?t~ٔVõ?sUÊ^ËÎÞ?ï)ÞÜLz5?"•
ìóJõ?€mYÖ¨FD?pêê}5''?'w‹ø}G?'FPÝð6?ï¹°ágl(?pX"œ0þ?8¬r
 ?1#ãs>–Ð?€ÎdDie?pkG	sƒAGN3FGL J0051.6+6445@^¼âCV–æ?þ3:ß¿À9†'•ùÀ;&±¥ÿÙj¿ÇùlŸÝÍÈ@MB¨ñü1@;ê€fí ¿âÃÔe>ëp¿â u¡<¿å®ò)伿ç:ӓÃõ@UNASNone?î8‡(†d'?¬œvʊóÒ?•
-¡4(ã?œ´Å|ÈéÃ?¡ðö£?¥Í|Žà?à\×Èd™n?Ó	e	f[?°7ÁøEg?¯# ^¨Ùˆ?Û8_ñ	ö'?ÑÎ:svø¸?ë™ÍßW¥?¦)¤Qú
Ø?ª(™Í&?–èãÓ?¶#†CBÎE?žu*LÐUR?ç§R2Žô?°ï©'¹o[?Þ1 ¢R?È<©Äk?ÍÀ{p8Í&?°BK†Q˜m?ï}Tz¼Æ?•VÿiwÕß?pü•ýÙ»B?~qg±#'?ƒb_ó'üÒ?ŽÒ9ã‹?ç½Us\æ?ÑUL©ß?¤š‹Ý9?¥›L°´r¡?Ëä&}ÀÚ?ÎÉ®õ?— ?'ußÿOC?"Ú>—˜Í?ƒqŽ¿n?›ÁZ»¨Ü?‡§$²ìñ?ìÉ:p‹¥²?˜ ²?<\Ñ?‡`*Pû4?r†>´Jê?¶Ê'0§"í?–²"áTá\AGN3FGL J0102.1+4458@_;6;%pÀ1ÛÇæ³þ À:‰–Ob=ãÀ;å¡ÔÑ~¿ðV+57ð1@
§òz†Xõ@í@Š´¤¿çíô¬²•¿ìÈÒÊÆ@?ʈJ´%®]¿é®þn–œËUNASNone?ï ¤+ݘ;?"úߙSÐ?S?WlÅ'?SŸœyµö?…o
 €®/?ƒÞñ±å?ïQž$1§\?"5³n–†v?v(º×Nò?~'öËm6?BóaÊ??'»U—?ít•Z€æ?šds›MæÍ?™Á^'âàð?ˆr(Bg¤A?«ÞWiÂh$?"5"˜p'D?ïgAؒ}Æ?ùý¹R]?3­ËÏ8ß?F²£Rø¹?'É
¿J?Ó:}"úT?ïޕ-'ú?k¦õ7Ó¦?BÜ,É/1
??‹nF@?l³Ç0þ?i©^|òÍÈ?ïÇ}G~nÆ?x5¢½Do¢?^¯¬ïò?]0EΘ{?t•q"ûU=?sÇ%¢?ïÁp?…)A2sqq?‡Bóì,?vEʂJ?"[xèWÀ?o"Ž©ˆE?ïåìJtÉ?bS'ßœöÚ?'"ù@©"?+ÆÁ¬ý;??h¡†8Åï?a€Zg2AGN3FGL J0102.1+0943@_Õ*¾ðk8ÀJ†«Oœ À9üÙ~‹÷À;¶Jt˜XQ¿çef#þë@
ÚŸƒéY@…*ÿ²þ¿ÓU3À™/3¿æ)"Á¿à<q—5Õê¿Ó14iØЀUNASNone?ïÅZÜyŠ?~ªÙ&T?4ËùÀ1?4r¸±x?|H}ùÿ+?}ã†|ÐBö?ï‰ÇKzõ?Š;¥ù^?fq~RÚX'?t+ l>¾?‡ñ͋"E.?"¡†"{Ÿ?îŽþiÒ×?¼¡Q6
	?ûÔS':?wވÉ¯?Ÿ?v
ž?‡µªhÁ,?î­Uö׍E?''õò}9?@®–¬•Å?B»''#&?¤çæ>'?'v0öÒ`´?ïìE´Û6?cÕ¥¸Zª¿?'ÇS¹µO?#Þf xXÓ?b=ÖhĜø?bú]̽÷?ïÚ¤("Çó?l2UîèÞ?QÁ¦àøP{?Qç˜_­?l{íýtb?fieÞ!ý
?ïjø…Hø?wÈ;˜yâ?}[ª)á?j\wôß³?†y°Ò«?qchª@_?ï¼ÿ]Ô؛?jåävÃÆ?(-¯°wÌ?D­¼•"¨?€_qÈvÔ+?j¦R²¥ê@AGN3FGL J0112.9-7506@rÑ.Hè§ÀDøûüe@ÌÀ:o5·qñµÀ;ùRÈ#ð À°§ø¬út@
m…6‹,n@`ŸõÔ-¿çÅùÛ	¿æZÅkY•H¿áªú_à˜å¿ÙúÛö,äÝUNASNone?ïÈM}œ?vXL"M•b?-sVú@ŠÖ?%(8ägŠ?zí¦Ð#šj?vÿ|³–?ï—ÉÎÞþ?†ÐÕË"Ù?d(\ê·Ò?s•5–œ?…¹oŽ2|?€¡Èì0Rù?î0z"‰Í?'W985 ?Žô‰æYvû?vãƬP¥?¥;5@kºj?Žü_F‡7?ïÓ®w{â?tà˜O¥VR>â'R¦R©>õWühEØ?v®C"
?tܨ¤?ïîLÒý¤—?`qáSHz¹?$-'§ùô?2hƒ‡>?`q:A§º¤?`%˜qϜ?ïݗ S?jÄRћU?P²)D\O[?P^{	
E~?jÐ…¹?dƅYt|0?ïU¯Z(É?{'è]è	´?|¨pG Þs?cwôql)û?Œ?ñT
Þ?wº¢">£?ïù4‡<Ç?E
Ÿ«È>«o¯'Ñ'&>¼8'á*ŒÈ?K'ÔhÍ?E÷Ÿ½§AGN3FGL J0114.8+1917@`P§æšÔÀE¯ž¾œˆÀ:•k/ùÂÏÀ;âCæߝŠ¿âlä{%vm@
1_C1ƒ@{] :¿ëḯéÅg¿Ï·zn¿ä)nDÅñ€¿â¿#ì:È UNASNone?ïÇkïÙ:?'ÒŠú	
ø?`üÕ³>Ò?wQ'Qµû?s˝«¬«—?u¬]d^Í4?ïPiTWp)?"åi'I$?q}ó)闎?{"
®:(°?'"Xª£ò?ûá§C˜?í±©-"?—è¦ÂØõS?›;Ò,?‡B˾í­?§e&»Ï¦%?'xÌÅö–?îÖPG|Q›?Ž'g"q:?o9Š-GŽB?gb•cL}? §bå:rf?)¼'hBÂ?ïì­2±5Ë?dö¤¨fŸ?E–û:@pû?K !#qöÙ?[Úø_—?bÙ¢
Ղ?ïÍ@A°ñÇ?u5J‡´$?XnéìfÊ?XµIR£HÁ?sD^
˜¦}?qê
ûO¥?ï0qÝú?\ÂXª?†P®¯…ˆ"?t²wµêw?ªtßÛ/W?s¬Jïÿ÷?ïÀjZU¥¾?hËQ¸‡ƒ?P#TPp^µ?>í§òŒ.q?{Áý°ÙGù?g\Ò@bœ\AGN3FGL J0116.8+6913@_L³åu:?@ߑæFñVÀ9xÓ³pÛ4À;04	t?ä§ÉJaM"@eQ5|¹@ à_Ñ¢¿æ` ÇJ×À¿ì°Ê!:§
¿è‹êפ¿ïýôf]›ÖUNASNone?îðÃÏ? Y½<Š@?‰ôÖùmáý?‰W1a™D'?•ÜF%'?š"6æ.
S?☜a)¼?ÌØ N:[Ø?À YÑê?µÿ	†¢­%?ÒÊw9"Ó?ÈHEº°{Å?é›êä‡K?®Ê‰_;?·X£'É?¢
vñZ?»ÈÆF(Œ?¥®eDݒˆ?àª9Œ½?³÷(#IV?É
ÄcÈ?°#c'Æ?Òó´¡?²>xê˜&â?ïpÆ=UdÐ?¯íÄfsh?|	-ö:]å?}ÌÞM§J?…ÉÙ¡s7?¯'–=†­¶?êj/@µQÜ?ÃȲ?®ôÜÉ4µì?«aäd'±W?½4––ý*?»{ÂÐìäg?í"²9â? ø
ÖõÇ?§éEÉߒ?"ë8{O4N?§´›I?–¿rŸ™^?èX«¡È«ð?¤»@yÁÕ?¿VÐ~)ž?žRõˆgI?½ãÒs''?žÐ#AÄ3AGN3FGL J0127.4+5433@`3:}ªÀËDå^³À9êÁþ<±aÀ;t»ÑÒÆ¿ä<™$˜'@·ºt°@B‹ÿÓ	}¿ç]Ñ`¥•¿äÔºLA¢¿í–úNÔé?Ç z^ò\UNASNone?ë…/çp´j?¿"¯Wq?™|w—2®u?–]‹ÌQ|Ê?½wbÞ­±?½F*[É)?íΉ¿=Å?¸Il죓?ŠÅÝÝOد?œòõÍÄeí?¬eì'쪃?³+ó
ì6P?ëS7Ç0ox?¨"nÏ{Ö?¦²ú"96ã?'Od\Äþ­?ºą;ÏË?¥H§s'é?î:îk¶ý?¤Ø"¨¯fS?Zf_¿ˆ¢?jËjÇXI?«}æFÑr?¤¶íÛm×ý?îÞ4‡àÎP?¥v§\gïY?xD™'Oð?{lƒ,u¢?ž8ڄ»ÿ?£feÁy'K?ï@x­$ø?¥Àr(-Ê?u',/®ýX?‰2¸x§½'?'§$»ƒö°? š¥®ÿw?îi:WÙt•?'aÛÜ/?'u^кm?€&†eðU? 1«<À|?ÓÀì÷?ﰚŽÙn"?yƒT»õ‹F?*ØÿÇTlÔ?/Ç_4và?ƒmøDŒ"X?yYù´J±AGN3FGL J0127.5+5634@_û
å6PÀÏbùÊ[ÙÀ9†}™ˆÒ¢À;V¶7_Þ¿ñîJ 	¶@åtìf;@°ª_d"¿á>ûù`(µ¿ì•
5üó¿åPS«‰í:¿ÊÑPŸGƒUNASNone?ïŸnÃ_Ä?†HÖ®Y?_…ú^¸?^XÖ"ß?"O$úº©?…N0ìZQ?î?qnú?°[Ü8H?Ëe©[
W?‰zmîö?§–¥©64?­ŸVê>ð?í—"©S? ‡_yEæ?›-f«F×?‰êÆÉ,Î"?°·éÙhŠ°?›gä+=dr?îÜw»g9?'ÍÏÅêIN?,kQW.?20Å!M—!?¢"Óo¢Q?'Ä%ŒÁè?ïÙáª[°?n§}›(ëR?L…]HÚý?Jŏb®?nüõo¿fÄ?kÍQÈź3?ï^°§´Ã?ž³¢úÙ_?mDr¼4?tÎã­ÚÞN?[-yë?še[ÒÎ>s?ïB&ëý?‰?ŠgI%¾?…¤'ð¹%?t7:1/Ê?"¥¯aö?…eébñ?ïÅf¬Ñ?iäŸ
;?
B
•YÜ?gÞ²3k÷?}ÈàdÊQ?iÑlu[³AGN3FGL J0127.6+4851@`!¸'ú
À+(iƒQX¸À:ÞC핚À;¬RLÓî)¿üˆà¡bç@Ñy[á}3@•Û_⓳¿á¨Æ0o›¿æ«2œ›'Ô¿äH-û)Æ<¿è‡S@]¾UNASNone?ïøM/Ífê?L¹ÅÀOo?2&ÞªÖ?9Þ1}ÿÛb?E·ÒW²?GÆ°ÏJÿ?ïll'ßÍ?'ÄŠ˜{µ¤?pòó÷ÚÕ?xÙú=?Œ…[Pi?«âßE?îï±LØdŸ?†1Õ«\?‡_:NA–?tݤæʾñ?–Z9j+ƒA?€Æï;ÚE4?ï'QæžýS?"Ip†Ú¶?-=Ä*ïœJ?4æÀjžq?ŽöDÕ<Ë?ƒåƒ+àÚÔ?ïü)!?€?>{™ª b ?"A'5\?%δ/©Z<?5–\aj¢?:Ò
Ø<{p?ïÑ&zàhW?sÏÈl RÆ?Wùìma?V³mä⨹?qˆÄÁì?p-ZH!_'?°PüX?px $œQ?tnoÍTöi?c³­=S?D·è€±½?g´i§*%>?ïç;"?\ÀGû6­"?§%?ÀÐQE¶Î?h€À#+I?\Ÿ+۔ÙAGN3FGL J0132.1-5340@rÀˆPœÀO4MUhÇÀ:‰š8ûÊÀ<¨Å†‡n¿áEÉ_ÒE@k~K4†Å@Ž#"ÅÊ¿†Ÿ
[sz=¿æjÉÍhþò¿æƒþ8ø¿á}ØÚ"UNASNone?ïǜÏ≀?u}åàüMÿ?`Ö!óbhK?aæËThiK?sƇ)"Ã?q՚ùƒu©?ïg‹«€ˆ?"PÚٗðÔ?p	ÛíB`g?}´GÇA-?Ž' ý¼ß?küé¥>¡?íRv4d¶Ž?›oþxh? ~Îݶ8"?V³"'?ªYÍÛ"w?"DãíwR¢?íðêSEwX?Ÿô1û»?roH?8iô?p™¶'v[c?®£qÆ­(6?žóP–±·ç?ïíˆc]¿Æ?]Wzµ²º·?C3øÄ5?D&¶ñkÚ?[`Ÿ"µÕ<?Wêõ¦Zg?ïӎÑ
Ï?s.ŀÌDò?UãÿŠŒzë?Wà&[âf€?p¿÷$WÙÌ?n#Gm}âÿ?ïm6ðæ?ƒïª€T?Ž¥Í&p?{«MW>Ú?ìQgv"?vØ¢z§Ê?À"¸?w–Ð÷i?QnŸÀY1Ú?C‰À<šÐ?…¬;ß^‡»?vÙ=M\:AGN3FGL J0133.2-4737@q¿'»/ìÀPü_oÒ À:/Ùâ_À<Ê~=ó¿üšg<z.Å@@âH_@¨è?Äæú¿çÇoE»©—¿æ¢Ißô¿ìä
‡Z°?¸K{Íð}UNASNone?ïÚ]ú14?u'¥›o܁?`·%Ã4Ó?plŽáa\?dëv."è?iœ2å«L?ï•g¸Ëãï?'™6hÍ?f`MoäÝA?zÁ/nŒ»?…
þp]á?‰ïcYÿkT?í«X͐[?Š»ŸÊá?æ»£X?ˆDiäN?¯"W8Ý¡?˜w –û?ï›DéWá­?‡.ðö{0ž?A¥t§?+C˜#N?‰Ce¾q?‡"æ5³Óó?ïé"öF*?iEmB±©þ?JP4êÚéø?Q /¡âu!?`HüŽª~ù?d—â°á?ïÞè-Ùà?qˆRr¬Y?P·™©È²?W÷~~FÀ?h¼Dܨ?iMŽ{ÊÐð?îÑîšc)?‹¼P+P6?Q1dÀ¸±?/iº¯Äù?—4i'êDq?"XG˜.°N?ïóÜ{k†6?TGB²H¼X>ÚZ§üùø>á[{ƒé7?X,®E`yî?T=K2)8AGN3FGL J0133.3+5930@`pyåŸ,Àg±j4À:
ˆß72œÀ;i)¾?kP¿áÞÜ°UÙâ@f
uú®@±?ÿÊP¿Î¹¸|*?¿è9@ÔB¿ÓÌ8+¯J¿êwÎkûCUNASNone?í²O'o1?®)Îð
z¯?ˆ"H{Ûæ?ˆŸÜZ²ž»?®ÒtÑj»?«òÀfü?ãÎlÅiñ?Ó·‹'O?©I%2Ëv?©ºôÒF?Õ:ÎvÐ
?ÑuDKo¦<?ë$­ßKÕl?¦¼Ìæ­[‰?²!Wíà?œ‹RÑU•?´¹x†IfÄ?žÜb'M²÷?ì%¼v­L?§ÿ1[ó?t]©¿Y¯7?på¬êb—?½ŒA±#g?§‡{óŒ^?ïS3<Ýæ?'Ú±Åh.?tU⊤3Q?u;
?"r?âÌ~Î[?êð8L`?ËFöZ©‰?˜éÐ.OJu?Ÿè7µ™—{?Á!å"**1?ÈbÏǼ?íñ­çj™?š
ešÊ­I?£nXØq6?"FFq ƒ?›·Í'aÊr?‰DlÛ9eì?îÙ=R4Äò?‡÷É»û?eú|: ©?UØZÂ<Ô³?¡‰u I?†€XÒKAGN3FGL J0138.5-4612@q<w¯dÀQ0Ý)4­À:W'hr°!À;õo|ž¿â
Ô1£™«@
ŒŠâq¥@|äpùg¿Ó1{©Ñٿᇜ|
9¿áT¯baR¿â¹'£¹¶£UNASNone?ï­
Ð"B?"¨2H-"ƒ?G÷QËn¼Ã?H˜mŽV'?ƒ=Çvϧ·?ƒç€Ó]3Z?ïf*€KÌ?"…eN=‰?pp†TË?~wÓ¨^…~?Ž=QÆ?N&…y?îj]N)•?Žs5 ?'&GšüΦ?~w°HÜ5? GìÃ`?†˜nŸ– ?î7‡¢ü&?™ßƒ=´ð?gšÐ.`Ð?cG·¯ó7ò?«¼,{?™CDT»?ï¾ é]ëÝ?±{Xê;˜?-ã0
áZ?*½i&Ο<?ÀqÍ]M†?±; l?ïԊŽíKÑ?rð|…Þ»?UŒ—­€Ò?UäÙÐð?pW'ÇnN?n{R®9?ïVÿ3Yý*?z˜ºé£Ü¹?†tXÙiJ?nlõÖï+?ˆ¹¾Û¦!?t1K
`?ï£-¥i‰?t¯kVf1?JŠälOã?='QW²2?…‹èhûW?tˆ‰íý9AGN3FGL J0149.6+4846@`—*0U2aÀ)ûԌ´®ÉÀ:K8ãv\À;œ˜È¹AÖ¿‹#ÔÛX@šq¾3Vï@õ `]7é¿ê±®B•s<¿éªŸlRŸÆ¿×K4Õ'lß¿ãŠò¯+ôUNASNone	?ïðWôç%Ç?_:"l^n?%¶™J¡?#g̗­HÆ?\®Ÿv»À?^0Y~?"?î7^ÊvíX?²&­c±ó[?ŽLŒã³?œåx<PA?¤÷²Äˆ½?«¬4‡3J?í
:I/§?™»
Bÿ"?•¹$Ÿ'À?ÞÕäÔ¥'?¬¦ÉùX¨?•—;ýî>?í†RÍ?£UÞ
Nä?}0ƒ£¾?|µ"7¼B.?µš†ªpÛ?¢:âN=?ïøE{?I4‡QÌù?|¹mÒ?ôûú‹éÒ?Kœ	ʖA‡?Gdz²¾‰®?ïqC°j&Ì?˜Ì[S[ô?ub1§æ?…©aN)?ˆýûj…_?+˓ofž?ï%WtÓ^?€!Æ;ʙ´?'
¯JmÒå?i90ÂNa?'N9¸¢7<?yôÐúªf?ïB>|Θæ?ë>¥sÁÀ?rñŒ:Y™Ú?aQB¸˜T¤?'ûÍUÇÎ?€ZØ `úAGN3FGL J0154.1+4642@`¿rSÍÝÀ-£Íi8À:DPXÝèÀ;¹—×øyú¿ñîW@َý@
Ð1Ü@j›`n)Ô¿çLܺß0¿â€w€ƒâ½¿ïÿËeªºå?ïýø£ë,3UNASNone?ïvž†#¬>?›1c"àÇ?hž&&Fo?pE)¨	'×?Œ0Ôî‹6Ë?™Fš"ö‰¸?ïkfÜÂ[?šÞ%8"Ò?r¹ EÌ ?ƒ·OX?‹É錃Øþ?"œÙÏp"]?ìY¸4±¯Ý?¤éI'5ËS?¢	*M‹?o}î½o?´19Æ»´Î?¢¤Ÿý£é±?ïÂHdÉ?…:²пp?"ÐRÕq?03¬K	xN?~•žM¢‹?…4Ò=ѧ?ï܋"LIô?y¿VâxÒ?HýGr?Q¶9zÜ}b?m5Œ.mò?vѯ§!hm?ïÌþÙ9l³?ƒ½;éqêo?\sB4?l¯2öµóÿ?rc³ 'IL?zùãh%å?îßö(|?'$¡»u8F?Ö#<¶?zܹ!k­?øצּè:?•ýI@ô?ïú.6õ	­?OÌ.¿ð¹>ËýÙéM5>æAò³Œ‰0?G+%¤}˜õ?NùÇÛ¹½AGN3FGL J0156.5-2423@i¿m	Ö¶ÀRÆÍÈuO7À:žr©jÇõÀ;äçW'Ž
?ÇÛ_¦r‰Ï@;-Ö'•?þ7>ÀZ#?à);Þ'"¿Û0š5ò¿â°¡$Ÿ¾ï¿ØdÖ°LUNASNone?ïë¼ò9Bí?[X
»ÂNÊ?/Š)^P?'¥\5›hÐ?bJ=n~?Z9ÞÕÎ?ï"hr/Gk?ûÏNY?iŽ¢£æ?wãzk`F?ˆ':¾~¸?‡@4¯?îÉ.Ы‡5?‰ÜɁ>?Œ`—Û®…ó?ww…ˆ ­?˜©Ùô Ðd?"QˆbT}ð?îbià!?ž…°€&['?pàCú?c?p6 š÷?¬¢1ZÐb?‰¦´«I?ïõï'ën?M+ŸïË3?"+ÔESæ&?qzüTr?QÜ5u*Ã?K^I˜[	¹?ïÙ:«~A?nÇ5ˆóŸ?S;;ÀJˆ?RšæòzÝ?m<·ƒù:?h"Vü[_?ïqšÀ`-?z*±§Ìõ?}eÒ¦+Q€?h†£'
k?…ïþâ?uŒêI¸m^?ï—B'ÝÎä?y]$rIúB?]g»WYÛ?QÔº÷eë?†'c×q¿¬?w~ç:YÁAGN3FGL J0158.6+0102@cpcŠ	ÀLÁ¯ ê[SÀ:1únƇÀ;Å;"ë½S?Ö¨j²@P
;§Ëá@wÑ߆7è¿ç2rÓ~¿íëMƲV¿1š°.¬G¿Ò'¹'Õ§‰UNASNone?ïõ!¾–?VñZÝSv?"_Ý?Ã>	VÑq?T½©€ê?V ¤Ãø̈?Xý>§?ŽZ¾V?fS%sÜa?vWŒt´?…ÕÔëü©9?†˜ò(À	?î&ÿÿ\ʏ?•9 næa?‹*¤Î"çÍ?v0Á#Π?¦ÅVÓú¨"?"C´ÖN^?îÅÁ)D`Ç?žûl'["?Na}½dpp?b"ç­Ì 
?£*gprEý?™ñÎÑï'?ïøüõÙ+?Mvê™·?eqéxb?`†ç‡?J%ÕVö2w?LÒþÌDF?ïÜh'ºe?n<±å'{?Qœ]ô¹?Rî"hÌuü?jÉr¨P°?g3YuŽ?ï%ëfëÇd?‰¼A¢'UÜ?x©Åk"æ?`æ\BòÖ?•!Π¦B?‰-êVÇù.?ïÆ»BX6š?u@ŠØ`QÃ?K~´"?K»,БR ?y0¾•MÃÑ?tÙ4)tcAGN3FGL J0200.3-4108@p`ì"h	ÕÀQ…=ÈK^À:o×½Á—À;됝T9¿åþi0O@Å2í<™?þüÀZxœ¿ï¤Ew¶ùY?êv–§Ì¸*¿ÞaË.žW¿ã𝫐ÖÁUNASNone?ﱊÖՆ§?¨¼ëo"…&?88A+{|?Z°
¾Ü´u?'Û‰²ªq?¨3Ãb&!?ïb5×Ó;&?'J2ö!…?q+‡a@‰H?x‡[`œJ•?ŽÜÆ\H¿Ý?‹³ Ú?Kü?îÜù1H'-?Œ–ã?…–o* ¶›?qÝÃW<®°?™•¢9y?ˆèÁò6Â?ï7†å%Î?"RL»àå_?|[X{R"?'=C¡¥4¸?'÷Ëå™?¿¥‰÷A?ÍA‰/?·µ§ø²!Þ?K ö|?']2⵪7?†m}JÈ?
?µôS÷£æ?ïÒ ]B¦?ráé+®¶?WÏØ^À£?W£Dma:)?pÿù´/F½?nç'Ãõ­?ïwdKÀ.?Aplµo?wÍ!¿Ê?d%v±¶¦?†@\rŽì+?{Á5Ãôõ€?ïÖ²Êÿ({?ku•œ}?Mš5í'?L,¨E©?póJ?2Rµ?i«#oqÙAGN3FGL J0203.6+1148@b°r\=îxÀG§>›A:À9̚`hödÀ;lQÕµ©›¿v¸ŠF|¨}@üçá¦#@·SàQäÏ¿å]Y¸`·®¿êÝÍç½g¿êÙ0\áyÏ?Лü,XEUNASNone?ï=—±?›Œ(ˆX€?iÿHs®òË?kýS÷§­‹?•ö¬ä?š#ÿj'˜?ïS8Í.¥
?¢9l
ÔÀ?rÿÍø¸?‹
Wº"¼s?ØóYÝ5?™ûâô]]Ê?ë'P6$Š?©Koø²ð?£'œÕ?i[ÁÐM?¹á°M~ý¦?¤óB×eãý?ì©_½!V?²/nÙÁA?jcê²O@Û?~(/@Ç¸?¹ä¥­4gL?²´Ô"‰"?ï®;{j?ˆd¾Ë¡6n?RžqEk²¿?ZVÁ-3vC?'S ±õ?‡¼®<V?ïÆÇHÃ,)?ŠGI?¹ÿ@?`¬IÎðÞc?z"éˆ?tF6˜ƒ?}(Ô?öÑ?îå¸M†=?ÒÇlùn?=Û70´L?zÆ[ҍMÕ?žD[WGB<?ŠíŽUœ(?ï_Ýu¼o²?Š—¦?éPÆ?H°x¦óÎK?RÔeQ!]ƒ?">Í|<iý?ŠMm—þ§AGN3FGL J0211.0+1922@brVWûi˜ÀCÓ<ŽXÀ:%S'^²À;²V´A»Œ?ÀV
1tu@
µ4¢žûÙ@•€r+¿à`3$ª¿éN·ñH'%¿âoÛ
 ¿ïÿH¯
2ùUNASNone?ï\4¨Þ9?–'-=[â?e'Ÿ4<Â?kWà:™U?'ÇJ›žp]?"Î}ë¬û?ëÞ]fô'ô?¶…+©=?§¦Þ £?¥÷V"S' ?µ€Á¿'!Œ?¯èÌ©-¹¶?êßՕ?º"?¦<(͚ T?³V."ç±a?›~YéÐ?µ«%5@?? äàÖN?環ÖÄiÉ?²
Àüy?±»ý|߆?¢ï×DÎP?È×>TÖW?¯B¹æz¤µ?ïÑC‹èM~?rØ ÊÎ5|?Q)(Щ/J?Tl•»LÌ~?sïðl$ó?o¯÷q?îбîÐà?›ÇBÅ›>?-oÅwÓR?‹hX¿i?—S
AŒI?'Är£Eå?íwl¨õ­?šî¡Mg?¦•º¼ÔÝ?Ðù1x«µ?¡øÞzS–?-À÷dLœ?í8]".S?–Å#£,Ç2?žP§YÃQ?…qÿ¸¾ˆ?­QÚ¶kø§?"0oõ¶nõAGN3FGL J0216.0+0300@d
\|ؘ³ÀJÌ~bÜn+À:§.~˜ŒSÀ;äȁäq.¿êàB&"èÌ@
!Í°!›@2@·¿êVbÉ_J¿à(³éãQ¿Ø2|mӇ¿ã7µeó UNASNone?ïíº@‹¾î?bė­†å?&("};£ý?#í:¾vo?`ã5ïÑÇ?atd	û‰?ïYrBpE–?¥,*øž"1?mm˜Æ 7?z.¯ v?'.
‰0?¤3´ð.ž?îi"†•Ž{?"!±¥¼Ù?ˆ*
'›è?sæƒ.r?£]4òý˜Z?'?µÎ?îíб™ü§?Ýÿž2?JÅÁ™mR?Lm>ˆNU_? ·ÝàòþÎ?«D·¡Ò?ïøœx¾z?M¹¿Ì?-ù¼ªó?qv÷Ö¿?Jh]üiÉ¿?LH¾ˤ?ïÔ3yæ13?}Gf,˜?TÈR|w"?[à_ _?p´=n©`¡?x5˜°Àô?ïP^÷ !L?[àÉý7?|àús|Ž?a±T‹ôp¥?àѹ Ÿ?|š4tÕØ£?ïÅ Jù"–?h?MQÓA?6@†ù¥Åï?)Q»üÁ?|Ò5_)?gúàiãL¯AGN3FGL J0216.4+0507@cÓH˒:ÀIà{ÃŽÀ:v¦%™½À;à€³Æ ?ÃT_Èèf±@5–٠ų@ë"ßöu=¿ãêRn·Ä¿Òë"Ì
¹¿ìƒh¯¹8¿Ø¼anô™UNASNone?ïÛ®˜‰?r>à?º7ñ?dÄßMñæ
?m&–2©Ñ?_=2+q?_JƒºgÍø?ï^Hˆ‹L?"ÒÑ£À?o|LFŸŠ–?{Q5"߀?GehfP)?—€@«a…?î&4-?•àFbv(?œŽêǒ-ó?Ž'"ѧÂ?žª…`bÒn?ˆoðeɬ‰?îšGÕ?™P¯]	Í2?'\Çu"ÅW?ƒXIÇ7F?£o)´}wY?—•;²Ï?ïòøÌk9E?aPSjŽPÕ?Gˋ'^Óë?PÛĪõý•?LQC‹@~?\ϧ/÷Å?ïÐÖëšÔh?t§²t?V"UÛ@èY?Z-ñõb,š?qót²&©È?oûÔráí?ï35À'h?ƒØVô#—ü?Š[·?~"èa ?ˆ² '‡–R?v>õh2R'?ïµ÷ë€äc?tž¼]҂?`àŽTOæ?T[³Å=Ü	?|ôÒG?r
ë<"Ù¯AGN3FGL J0221.1+6059@`³"¦óõ0¿bÿfÁÄʺÀ8Ç`‹[uÀ:Ž¬ÇsÇx?ìy­
U@ºOÌñà­@ts@i|›¿è«¶݅,¿è$ŽßE94¿ë} ÝΰZ¿ïþ¾¢ù¥ÚUNASNone?°èf¿fW¯?± ®}—µˆ?Á4Öÿß&?ÀëÊøÐût?é¢åò|x?Åg­–Ú*6?†«š=§'?–¿'ÙÉñŒ?Ñòžú<ص?¿%Zh½?權ÀŽ?ÀËASÕ?Ë÷ÒG~;?°Dл*H?Ñ"Gùq?²³¼BŠq?à€3Š#¸?¶8Œ¸ól˜?ÀpJú¾çK?¬†äû¶§ï?Ö]ì‹?Iþ?·ìŽÏ?à´öû°¡.?ºüe§àÀ[?¾¿¿nр!?¿Ý¨5X?Å]Ÿô¸µO?Âå¶J ×Þ?æРn2I?Ë^âäfG? ­†B`?°£Æ?Ò7µåeÜ?¹@ð«¼@?åÙT"¤3É?ÁJ5¿eÂ8?݂2\ñ{?´Ì4ÒÖ¸D?ËAµ˜RÈ?®P¹é¶¶?ÔÝ?ŽéÅß?²†}
@5?Ί­è?³.eó=¾–?Ó&¶È©|'?­f "vÏR?Ý˽qÿ»{?´aPš$ÃMIXED3FGL J0221.2+2518@bjª¸¥Î[À@£
ⴖÀ:LÓP0šÀ;à { ŠO¿Ç±Ä'?N¹@
³9Ó¶K?þø…à19¿îÉôYo?à¹*,q£¿×SŠ^ƽr¿äÁ¿z÷UNASNone?ïãl`rÓÔ?igU»™ ?;ŸIhÔà?9ûwa•‹ë?i0‹¹Fk?gÙ4ò'Ó?îu™»,Ã?¤îõR¾C?‰HÎm="?ˆèžøCÂ#?¢T0ÐI²e?¡ŒHœR»Í?î§ú+ÄmÇ?Šƒ9»¬?‹lcšH?x[ˆ\tK?JˆºNE?"¼'˜¦?í¾ôW*^M?£›n6®?™zzWz‰?'ÈŽ'¸*¨?§"ýRÂá? l4!=éû?ïõNA'­¨?P
ÊÛ?(OôÃْ?&
Ç÷AÛ%?RY~¡p¨Š?MFܼ[ï?tª]?ˆ¬ ƒ"÷¶?na}…Q7$?j·Pg?'þCs‰?"ÅtCÛF?ïbúqS\ý?w÷‡!bà?~Ò)ðù®«?l¶yì¡í?‡ØN«Ì±{?oݏj$6Å?ïf=8g?€…Нî?z`íyW?k"°ØH®?‰@;áœu?{P:'á"RAGN3FGL J0221.8+6138c@`®›¥ãSø?ä8찗âàÀ8íŒ- L;À:9GMœk?éñiþ÷A@O‹8Wà<@[Ê@«kÔ?ïþːü¿êÐÛøíDÅ¿åoKKq²9¿êõ1ÌńÉUNASNone0?|K¨WÊÆ?…h×Ö½¨?§ç'›´¬?²/–ƒ€ Î?îNZ6_ì?³Qç(Û¥ß?›pÜö‹n%?¥n'VtÃÜ?ÁQRœÉ¾"?º);&‹sÖ?êÐ$q4±Ê?¿¯qîÀù–?Ŏ³÷é±	?©'™Ë8e?Î@H1>ˆÉ?°å˜ó"Ü?ã@ö?aë?³Ê[	Ò@ô?»Wt¤b$?±ý"˃´q?¸Fð¯t?ªÔÄ=â,¾?éƒ(¢?¹þ«ßDÞ?p{o­MÐ?'~™s9¹?¡Z0`
¥Í?·8›pìù©?îÉf¼õ?·Ì©
ñSl?±þî5ÿː?¼£ap¦u?Æ •¨.™?º.%¨í/Õ?è7üÏ&¡Þ?Åù9ÛKžB?Ïõ?ÙEh?°)[k*‹?ʊ@U…˜†?­S,|ÿ'Ä?á`ôMU"?³SÌS1)?Ä«nЏœ?¶¾Y"5S?½ü['Þ%?¦€@…•Ño?ç9‰Ä9€T?ºTf_OTHER3FGL J0223.6+3927@a¶¼œ#¸À4;>šo'À9Ì@Äì-»À;À¬ôÀ0Ý?ÙlÑYÏT<@õ"m/®C@:㟢J¿ä%,º°´¿çS$͔ɿ䝻Ýï½p¿åñè–	ŸÅUNASNone?ïeLÂÈ´\?˜Ìëÿ¸Ÿ?‡4É0A.?•'{ïgƒ?%4ïØ3î?}1yi?íLnD'g?ºÍÒ2?
šƒf‹×?§ »c"L!?¬º;ÞO™?³>-Rœ?íÂ‹žô?š+¯?Ï÷ð?šªL@᡺?‹ôjýM>?¦Š…ùXæ?'`}»?ë~%²A±?¦ ÈÊÐ…?¢†n;§3?"xcW×ò?ºËѲD_?£'mø¾Þœ?ï\s7Òv§?¾Ù½qÌ1X?''ºQl{¡?½‹"%¢Y?gvõiËä?"ÃóÐÀÎò?ï=/Ége?Ÿ}¥Þ|?þْj"¶?†÷çþbŽC?ZPu¼¯C?—z|Õã?ïCo}«?e	èÊ*?…ûã¸7º?{‰LÞ¹þ?‰@dî…ô?nÍßTåcµ?îÐæ©å
®?ˆҜòý?/~ۘ»¥?rÑÞX_ò?—KkPj'~?ƒ')ýŽèdAGN3FGL J0224.1-1846@hŽu:>À/ÀPÇÖ¡aä÷À:t˜XPúÀ;á÷Š¸Û¿Ë›éɁ@
Ä)Ùî@3ìŸûÞ]¿âT³æÌÓ-¿éûAÝ΅g¿Õ+s¢JSq¿ècÃUÍ~UNASNone?゙õŠAs?~½ºµQ?;‹Dö"n?7}+ÿ[øÔ?~÷Ð݃Î^?~ñìÊvº?ï0ì|L?—bò¦k³.?wÚb.Š?€±ôÖ¢?"ëý[äA?'X¾Ç¡JÛ?í•À æâD?˜}Þ/Ô6¬?•'ádl7Í??‡ŒIµ?¬?[¿×?"SHݺ?íp%D24?¡!"T"\^?tWÚ¿Ïf?q†]m̓?³9X4@!? Ž«)C?ïíÎb²ü?`%>?a-?'ÿÄÃög?$ì`Xg¢?`±¡Wü
?^÷Ó:î÷?½¸³?z§MôÃùw?`Èò?`·ó<V(?vJ0"ä#d?te}"Ñe­?ï0l¤w™?€¡‰^'Q?¤Ì1Š?jx
ìUÈÆ?' €,é¡?yHÁy*bþ?ïn쓫\Ô?|u½Ìr'?d»ÌUuÖ°?S˜Á?Ãiî?çòåP?zaN—TJAGN3FGL J0224.4+1615@c$÷QÕÀD‹·¼]êÀ:M®ƒ5ªÀ;©ãîQÓ¿ðò€Á1@±Ê]0ݘ@=½O¿äý×p·ª¿åË¥Š¾Šj¿ã.z:Èl°¿Û7\.nUNASNone?ïòJµ'a?T<óûéß?-¶àm³ðÕ?&C4âÁc?W³¹è…ñ4?S%ùÇ­¯?ïŒbŸ•ñ?‡çy²"³??eë¹p?s²g®oŸ?‡l•FÒ ?'0k?îÙªef-©?‰‹´¾3
?ˆa΁KÓ?rÔîÝ­j"?˜Ä'hŠ	?'è»ÉLî#?ïGQz¤"?†+³R.´?+¶õòdÂ)?-â…÷aÍs?–çáuÑ=?†úùÖ§3?ïû	ÊjX?<r|Dý^Ö?‡ËÔÇ¥H?Ž°Éó†ˆ?@'Ýh¶±?9ôñٟŒ®?ïÚ󞝺f?k
Cf6^Å?Q·ðÊh{?PpÓ6ÿ1­?l0hÄ·Äñ?eNSô–ŽÑ?FDKÎ?kÒ†·
ä?u¿sÐÕA?_?ë[ã–?€¶¥7l[Ó?a¨g›¥L}?ïÛf¨;Ú?^K
Ÿ?sD4ò?¯œ
{V?r3V'´®?^੘ÖAGN3FGL J0226.7-4747@p´Ú¤ü¤+ÀO«ud0+À:²Jj‡À;éï#8ê,?Ÿ´Ð!ƒý@
j´©ÀX@Yc_uÜP¿êzŸ6J¿é¯
Ñ₹¿æU·A ¿ãqÁt1UNASNone?ïßï<ä7?iÆC·i'?>þý"MË¿?<½ÇO"?m1%ŽU?hÉþÚo±l?îËYûÒ|m?±N£V?…»|ƒGî?œ:|oë‰÷?›¶ùÊÞjl?§î}›¨?í ¢Ú,~?žuoʾ*?œ_ûh@± ?‡A$w`u?°¶üŒcF?™áÑ·?ì.o-y#Ç?¬7qtK&P?'ªfºVúú?rWHVÔû?¹áìæêý‡?ªDÛ%yò?ïê84`?žs‰Á^?*¸}k¦
‰?(…(Öù½ß?dO@.<ç?ž¥Œ?ï«¢w'˜?•ƒðq	!?k(Ö ?…È$ÊÏA}?|š¸ç¶\Ç?‰aIÝHäÙ?î÷kf»v?"*?O"Y?ˆ¸…ÖÏ?ux¯íڕ¹?"¶\
–c?}åÈ-@)
?ï8VñSiß?ˆêˆ4òo?v¡‰ÇþRŸ?h'Í‹± ?"L¿fÖÐf?…&:pLíAGN3FGL J0228.5+8213@_"âëC-@3ÿ—þŽæ¸À:INþjÕÀ;ÖYjÕa?¼s¬h@
Èé>Èg¸@,( Z"t¿è§®K=§<¿äø'÷ŽÂ¿êë™ëñL«¿ä³°Šæ'UNASNone?ïӄÛW»9?t²˜¯±?cp]3'{?dqI¦­F?i
Ç ½K7?lj³?f¬?îÁõÔê
á?®'Ô˖8^?'R…‡3¨ˆ?—È©£ÁÒ?–n¿ÙÒÍJ?§[Ø°ë É?í«ú­Û\?š8é󧖭?™ÑØ)–41?†Ò·Áy'Ï?¨Wi›­-?"ô³~n±>?ìþVÌYN?¦ç$ñ3Ûæ?¨µP
+?Ÿàëô¢'5?®JûC0@
? "a–#ì?ïñŽq·F?`G™Ï ók?G
3;,NO?PH3×4š?Q\'ò—r?TU$ã¤Ö•?ï£+ÿ•Õr?˜Fô‹K±?sŸŸ6q›?vŒ'Q®>Þ?zÊa])?‰-]Âd$S?ï!ÞäžÇù?ƒ›žRx4P?‡w
œã=?vVùò®ãu?œáÁ‰I?{¬ºáý[l?ïT¸Bjø`?ƒ7Æaíñ?""€Ë¯zÞ?pïewÙÎd?†=n™'m?}0ÎRS¡øAGN3FGL J0231.0+1302@c¤pâÁ*ØÀEŽ'Ð(¡àÀ9ý«®o´À;hÞë0¿ðXþú~@À…Téz@b³ ~O¼¿çV]Ÿ˜a5¿éZ^÷˜c ¿àÀIcÌ-@¿æqâÌÀUNASNone?ïóðÜ»F+?WÓ0ܜC²?)=V"­Òç?+N´Î)ºÆ?Tö›GW¤?V'hJQgé?ï€ôݕ¥w?‰¦®N3I?gïÿDTÖå?sý-2«z?‰ÆÈÇq¨–?")¡¼?î‹2Ë.g?5p8±©?‹æˆ{?u§E2ÊçŸ? T‹.³ ó?‰þ
‡^ô?îôQ¼hÚ?Ù›òwG?@ŽÉ-œJ˜??ـ:—¹? x©–,=?T'f¶¾$?ïüí×ù?>ÃàJq(?8cLf?tÇ¡R?9¢zŒXùš?:ò¯3¦Å"?ïׁ~(Ð?m'‡¯æOé?S8äD…'?Qp	~@'?nâ…(šê,?g z|ÑÛ?ïy³¹ð?rŸd'?xÈ)"XÝv?aáÇ(¬?….üýì?m7=*ñ+å?ïÇc+svD?gãjxÎ?'Ù:LaÂe?ÖýˆXT?{ i;Ñ?fËEñÎO^AGN3FGL J0232.6+0646@dNÚfƒÀH¿‡iì-À9öKµ
8hÀ;µ"Ô7û?ë*¬K{I@@ÒMë@SáÀNå¿çŸ?åŒü¿æf ¾;x¿íkÝxG¿ê{çNz¯UNASNone?ïU¢F;x§?"úõ­€Q*?Œ&ZÇF²?Žñ/÷wAì?|â'qBìC?'W¯[N7¢?í¾z}äK2?°_c<æ:\?"3ßq
`?™–	 ?½?©þhjìjÉ?¨(–Ø6Fë?ìŠP‰ìc§?¥FD©o}ü?«Ã>Œ5`"?›ÇÕFañß?«—¸Øtö?™Ùƒß%È?篓sTO?³ˆs®,á?À\˜-#ú?¯å•í"éË?Àå§ÉL?«º¸»BÃ?ï'DS{?–¬K,t¦?……žGкr?'CÃw"3?sÒ·®"·é?'Ây뉆?ïMg2On¹?–>>¤¡"?}T~¹AË?ƒ~"‹_ëˆ?Ž‰"xÜÓ?x"âmÅ?îdÆ#÷g;?•Âm'¢LÀ?›ÀN¢?ŽƒÝ$×ì?˜b«'
—ð?Jâ;æÉ?í\=[çB«?™fÛi8Kù?©9̈&?Çòº Žü?¡]¸£è+?q÷ù}-HAGN3FGL J0233.0+6237@`Ê8›R~@(ŠbÄñ6À9h>­º¹À:²pSO2¿ç¯`Å"i@…&ÉB~«@XL jÓ¿èl÷òaÔ(¿ç˜Oº}iã¿ì×1ú™¿ØÃîÓTUNASNone?í9Äè|×?··ü_
`ú?¦Ñoi‡gš?±:â:£õ?¥$E]?­"^|z3?åedr½¯?Ôä˜à%?›4µþÏàE?£ûƬ-b?ӁëºE-(?Óä~úÔ>?äÒó°™îÝ?¹8—=wC?¾‰Ká³l\?«jÁaV)?Ío‹J˜Ìâ?³Î¢YƒÓ?êEA}?µ@#±Šý?`bèæ/Š·?dD'H†?Å}_YàN½?´ÿ@!µ÷?îm<ݒ(?²~¦ñÖM}?™/ºòs";?«‹ûCV?™(©Th0B?¤<¬É@3?é9H"—¡ó?҇zùªP?—ݳjt>Ë?¡T²Á«(?È'D‰ê?ÐÛËN-ƞ?ëL¾}1aª?ª±dXȂ¶?¬ÆB'HWã?ŸàúTA?·6êÌtß¼?¤FˆlÎôë?î7Ü;?š@«SÆʬ?B6à~o£W?7Î#Ôm?¯žQѾ{?š+3a5·ãAGN3FGL J0234.2-0629@f-ˆ¤~ÏêÀMf^ê–À:ëLÔÉÀ;ÚY§;BÌ¿È´• ˆ³@÷;á,«?ý¢~ðuô¿ºô¿§¦€¿æqô%‰Û?Ÿ÷*|'T¿Í†•'˜UNASNone?ïïA¦éc[?[|Ô?
º5®
?ó))b5o?_ŒÇÿN?[
!»je?21;È?ˆ4S<ê¡\?c¢àÖt4h?sñªó£A3?ƒð{>ÃìË?'4E^qa?î¿îC®Å??‡[`á²±?ˆœöòð_ê?sj–öøׄ?›³¼÷Z8?'šânõ!?ï	96yÜ?'Ìiœô}?4﬘–†Ú?Dµ6ŸÝë?ž…wÅm?'¶ÁÀ̆?ïöD`4Ñ¡?H#Aé"Õ
?¥P/—Íç?òز‡/
?QŒê"ѵ?G…U"î‰?ïßAjÈ9¯?k…ŽÊ?OüþÂ+??Pxé—Ô­?h¿UwJ:?eÇ:=ï?ïj‰"¨÷?sæÞNßöó?|IKŠ¯QU?dx–
43©?‡T7埁?mXn¬jà?ïÒUCº{?g~ù,>³Ø?2‡Š/5?0ZnI:v?uÏÝcÍù«?fשJÕAGN3FGL J0235.7+5647@aC¿rq7À	Þ×ü«·©À97BL«ª=À;KïW;P8?žô¸[ö@nȯ†Á@Û©Àƒ=b¿ç}D®-¿å¿SÞµ"±¿çÈÛ$¹=¿ìñډŠUNASNone?î\ÈоÉÕ?¦-³éY¼?£'±€¥‰?¢ànHÀµ©?Šƒ‰	d—?‹Ýà‡jÃ?Üä+2Þ¤'?ÒÖâ9ñhc?¹7ûY}å?²vÌüº©ž?ÜÍÕö¶?Ñِ"‹?êåÐ0{ë*?«$jÞKo?¶ÎÁpŇV?£"ZÀ7_Š?²½
8Y?›º˜¦E?éԁ¶gÊX?¤÷
Z_Å?¦®L€öš?•ÝÀs	?Ãf%'¥x?£8´3òÍ?ïeÍ܎®?ŸÈsœâ?™ Áu}F?œwýÌûÄþ?{L¹üë?y¨ã¨JPJ?çGI;‡?ЧúÁå˜?«–F±å?¨ÄL?†™0?ËýH[ŸŸ(?Ì ×Añ?íÁÀHýAV?žâ¦ƒ¹"?¦1nÂ=mB?–·[mÜHã?›edtª?‹ѺÛ#K?î'—7ƒi?Ší†ÔæŽÏ?‹ÅÓØ[€—?uõhE8lL?§–péN?ˆã"¿ÚÛ_AGN3FGL J0239.0+2555@bè¬1&éÀ>ö]9–úƒÀ:"Ë@ÒÎÀ;Êry\ã¿ÛºI˜át
@
[,µ•£–@~¸`¿é)I8òԍ¿è—›‡…¿Öïòª	±ã¿ÖaÀ~#¶UNASNone?ïéèK®T<?cøŸ˜²?"_.ζX?á±»úv?dñÁ¢Æï¶?bß¿%–ÓÇ?ïJ׌™Uý?œ\ß%«:u?uDm"y°?†¬\å•7ä?'Só$ØÛ?"TÂÛúj©?%ÚÒk?‹Ž\U"§¯?ˆ+ë£Ìô?u PѬk?¡LRߍÿ?ˆBó
¶ô_?î.Lú.¯Á?œ\H¤n?WÝ{ˆÆê^?a—l<5³?¬\DƒÐu?œYÕ¹yl?ïõÂ7s?PO˲áÀ?÷¡4ý€í?ò™=f"?S÷'¢A÷?O[ò®®Šµ?ïŅöy™t?"^"¬ð6}?`6ê^¢?qšÞß
2?u.éÊûæ'?yBÜ&éš)?ïX!ÂÐþ?z†ܒ;N?|ºIT@?käP‰ö²?‹šjÎË1?u![¿ÎG…?ïŸsó9?‰?t>'ÎØwq?L6f 4º?CDHG¥Oå?†_œÆëN}?sŸ;î8omAGN3FGL J0239.4+1326@cæ_ZÙjjÀDÙ5C®«zÀ:
¹üæpÀ;¡ƒB??±¿îÄ×,n•V@v­Aí
Z?ÿìe¾ö [¿ïMQ'Ì?áÌD' ñŠ¿ácH7¸dF¿ãwrt³þUNASNone?ïö%ÛºŸ?OÑz>¢z÷?/îI‡4°$?*Ø*–@?OmŠL{?KÈ[ÑÀ¨N?ï^®‹q?¯ŠÚ‹þ?oV¾8ñt]?vѓ…TOz??VԎgU?Œ{êõj?ï15›Ý?ƒI'BÔ«?…æ¦>wó?påyœÇ?'1e÷­Uv?|y|öÒ+?-¸?"Ç*݊pm?pÛ°°+•Q?t³1Ç(˜-?—Ö1ºý?'ƒ'¯táÏ?ïü:$Wçâ?6/-Išb?é6€õ"–?À^Îë?7t'ohƒì?3Ô¢bϱ?ïÏâb؉¼?r÷Sµ¾ü?V¾Äl;'?Ræ
²ûj?r_Y«a?pD	r¯ê?ï˜ÚƤX~?m(î	Ø á?u¾Á¯'¥?a]ä‡2 ?}ԆÀ¦?d("¿É2?ïÉw'ÃiL?o–'q
á£?AS:ð'èµ?@ýÄú&?y×#O-?nÃXM× ÒAGN3FGL J0240.0-0253@eÓ0üø
ÃÀK>ýuâlÀ:T¢Bµ‡6À;ä™/ŽÃ?è™SèNL@­Ô°p÷@€Ì_iœý?ϧïâj\¯¿çWvÜL¿¿ïÔFxVË5?ìý["KUNASNone?ïù›~v(?PXÖ[?@ï·Pæ?FñTöQ?7eF}«8?@͚LÛ¤V?ïšUÈÅà?'ès¢Æ?dôó¹ ø?xºj̈ùs?"-Pû ?‹}yáê?î
"='¨?š-¿qh¤¹?œÒÞ8ùÔi?'X)üe? íO½FJ?'û%Á(Öm?ï'
rägã?"à'pÒé?Hu®_°È?i¼ƒ>?‰öpÁýõ?"]»;0~?ï÷ˆÇ(6ð?'e‹?Ѷ?,TñbÙ§­?65®˜¾z_?Jǧ¶YÖ¸?'`iˆkA?ïßh³ü$?mzZ²#¹N?P\h#;©?Uý}ò»?hiÓQ½_?e .¾˜M]?îê'.n°ë?'­¯X–?'ìŒj8?‰2–ãÙD?'§Z>¾@h?ˆmà¤Éb?ïõ¾©Ö?hèoe°?•_-<ˆ'?B‡mÒà!Ç?S-Òèó?g…•Ä–DAGN3FGL J0242.1-0534@fS—c^t*ÀKûà¤&À:jùYó']À;ãåÇo•º¿ï²	Û~Ÿ@½§¹íÍ@×è€\†¿¿é`eŠÀ°+¿ä.ðÞ¤æ¿âTÂÝé2g¿ïÿZ=†UNASNone?ïç…Ô?hƯR¸é?U!Ú%¾ì?Y.*»å{Ê?[ÓÿýîÜ+?b
‰®°{4?ïsï^z½>?W•r€k™?m<ïôà?y4rãù?l?‹´ìsj·­?ˆ¦æt˜Í$?î)¹ÈkÇ­?–Ðvñ2"? R|Âȳ?Ž3•«8؃?š#Ít~ó?‹ráŠNA?ï)$³àäÿ?"rì=?\áéS¡?aõN"ö?™‹_ÿuë?Ž­çUûdY?ïõ%*ºq?S§|fóöþ?Ef7u[;ö?D¶s(‹é·?Fm4—æ
'?IÞlLƒ<ó?ïՐ©—#Ú?q#ùŒ¤å¼?UlÐôm™?T0þ
–Œ?o¸î*÷Ô?k.mŽ<[?ï¿?ùóª?…Ó>$)µC?'az†?ÓÄsDÒ?†MúÕ`Ԉ?xþ-†
È?ïÔ½¬è½?hÚX+ˆ??6¤ÄÐýŒ,?6™«Ä½‡.?t6ÝòJT?hHD;ŒAGN3FGL J0244.4+4745@a»C¬ÄðÀ%Ø?³t63À9ە+uϐÀ;©V)Ø@ž?óƒ#Á%NÄ@]¦^y(@þ€[¯ÿ¿èN›c?·È¿èÚç¤m¿í'<«WL¿ïþ-€IoUNASNone	?ÍNügo$ü?Å7Iv?ÛÿHbÍÞ"?ÍúÍÕÐy?ÕY9iz`?Êzæið£Z?°lZQà;w?·HŒÚ‰?䨓O± Ò?ÅÍõ°Š¬?ғÂËÓ8Þ?Ãt†(šö?âŽmŽxÔ'?²YôåÞ?Ό_æ*Òù?­Ú"©U×Ö?Ç9éßñÜk?ª=Ê·œ?»%!™û
Å?« 9?èòúB®?¹…õ1vÃÌ?½J–•òßË?¯xšLp;¿?Ôa@¹Ðé	?Éí¹´õž0?ÙԖFö+?˦«ÁËx?ÑÊ(ÿ8ëë?ÇF;)Ä?Íè2ƒàʱ?ÇK4Nï¯Ù?à–Ï'è/Ý?đ¯¨­;k?ϼp~uÚ?½rëfã0^?èzc?â»?¬ ›Eµ#µ?Ä=û×Ð?¥}+ÛÃ88?·üìež‰?Ÿ;£N'?Ô3üõb?±6Ѻ²Š?ãy+³ô?³æжQ»S?´ÒrÚç7?œü "BMIXED3FGL J0248.4+5130@a™
9À<ù…'À94´7ª'À;Oº*2Ùq¿Ð籺¢¨·@ûD¸Ã+@‰gÀ-­?ÆáëRôš¿êEØU'_ü¿¼e"¤7,¿áW£UUNASNone?î?û"+"y?§ÉW{«¶Á?q†´
Q?pÍùÙ†æ?©ÏuɅÅ|?§´›ë'ç?ë[ Ûé[Š?ÃÀⓈˆz?ž¥š–µ1Ò?£ÎÖØ
??½y'yP	>?ÀPƒG•d?ìeÝ_A.?£7¶µ?.?ŸåôöhzÞ?‹"VïÙtÙ?´×—È\p[? ³çÌ΀?ç÷M#Ñ?·u¢Æn?€3cÌ,?P/²fj?Ï"˜=E}/?·€W:ÒÎi?ï;1ΚF?•o1SC¦?m+]WG¤?mÀÉ4m2?"ôs_@A?"8;S[~?îf—g1µ?°®üê¥9†?‡Â'M
6?¾0·3ܜ?£­Œ¶Ib&?ªmoîE/™?æU›#?Ž²Vý|h?ÓÓ8lp?~Ö ÁÉ?šæK°e`?ˆ/ÐD~ô£?íN³æ24Â?ŸD~-ë?v³ž‡mÏ?gÁŠ"—?´&î5»?žj™uJAGN3FGL J0251.1-1829@i;ºKâÀN•6½+oÀ:¥?CÄÀ;Ã}ºŠ?ìG>^ú%9@
b›«—ž?ùëÿ0ø?ïÿ9Ã^ÿ¿ïÿô	N*?ïÿÀ¤Vt¿à¡âDrªUNASNone?ïj½•™§(?ŸY4ýø8Â?5ißÖ!ø ?79®ãç¨?'R¥ËHk¾?ŸL¤G?ïH·@•é®?¦Ê¥?À	p?tÈØÚÍ'n?‰R胂C?'¶á¿RYÍ?£a	»E?ì¦$,°5?£b_Ág±? n'–Ü?'dò–W?²—ÓŠ,ôh?ŸQ`R¢¥Œ?ìõ¾Of¼?¾Ò1¿ÚdÕ?f¡ËŠ4#W?†¿ê·§V?·œÿ,Tù€?¾~~±ÇôÝ?ï"bŽB9?"ÄÜ3V ?>/Ðh?<ó
=ܪÂ?‰ö²ìYL?"§ÁûbŒg?Þü¥-?ª>R>Cæ?uîÂç­æ
?'âÃÈÛë=?"§&ÝÕ׺?¤Ö¡x:m?î7t'Ö+?›uÕÝ&=*?";‡á"~·?ˆû½h:Wé?¦.ÄÄ­¨÷?—n³Ñyþ?ïNàiÑn·?žóQaj«?t˜éb[7?†Ÿjn&Üà?ý¸hkî?™jCsOáAGN3FGL J0254.2+5903@aDèh3Æ¿Â6év&À9Rk–QÀ:Õf££×?w0Éraˆ¼@­ºÛ³šw@D¾@Bo¿ä¨ÞI昿ë+`Š.m¿íµûxT?ÔÕĀ€¡"UNASNone?ÓËIr˜V?ΕÌZT?¢S'´Û?¨îh½~‡7?äù}KÁ?Ðj¶_ֈ?ĨŒ9w)?Ñ*v©³ ?¯‰ó'oæ«?³üÞA]I?èÝ=¹° «?Ðãõ°NY?àß¡g] 0?º­xt6"?»<¯•¦½;?¥Œ€
!?×q'KÜP?¹ÅüReAg?齋hÿGô?À#ÚOä?qüT*ÍÔ¢?"²=áTF¾?ÈyïºãkJ?ÀÔ¡qC(?àžû€
ô?Ðö/ëÓç?!Œ2LE?•§Â
ØÊR?ÝØü—L…?Ðû°ã«á?Ð]MoìÄ[?ցF°|_?±vü~'Ã?­Âðݦ£h?墖h×ú?ÔɅ±\?èõlK¶?u?¯j¨-oʟ?­vñ©õ5?—äÛÿs&ä?Ä̒fÒß?¬€€@r¯ø?î;ò«È_?¢Q‰Ï:ÿõ?SYØ4É.1?\IÔî¯ú?«¦?¢GÜ©öŸMIXED3FGL J0258.2+3555@b¼§›ºÜ
À47ÙUqKÀ:({_ïJÀ;¯è?ïÚÀÓ$‡É¸p@
†ú·Šñ@àÄ *í¿¿éÃG†Yÿ¿ä {Ó·'¿ïûbd¬°€?ïÁ˛R	UNASNone?ï›9Õ¨'?' ¥ÕÑ©?cè"Äæp'?'[Ô'?"EW¤uK?‹ª`1@
?ï'&&kŠÏ?NGê-?j™¢Í?s‡³Ìvi×?"ö6,Ö°x?‹ŽAÂZ<"?ìy¤>Ê?£T$í•Ý? ¯Œšä?Š¥$¾?³ÛúSÁê?¡:nxÊZ?ïøxg?bùÝë84>téY\Û@E>¢´Y
=a?NêGë˜+?bøõ­hCæ?ï°@òõ'?²{POY?và1´?°¶€:ð8?q®'!y?š-þ£Û?ïÙ4¿zSÙ?r>AL-,—?TÛSþ¥Ñý?VÇmŒV"?l]–~-ò?k÷v"AÉÉ?î°4k ¼?Ž¨¨çl?Äñ¢tR›?z®
2 ?›ù¼{
@?‰÷ÜÇ ûÔ?ïÿhî€ü•?éØÁïÂ>.D(Ą>;¶+<þ?â&cÓzØ?éÕ:ÁÂAGN3FGL J0258.9+0552@eW¡"úÖËÀFk	cV®À9¶3ßWÀ;†!È`?ákÒ]Ä_@
KYN$ü@ÿ9À@!ƒ¿à˜[êȜx¿Ýìß@0¶p¿á+µ¹=s¿æÛì4£"UNASNone?îâe="[?Ä3žN?x™NióÄ?zÍû¾ýA?¾^R¤?š8é3=w¸?í[`áP?¯æ€ÈªbÆ?—£ÙaÑCd?–m­*栘?®xQV;?©Ã1Ž/'œ?ìÿ¹˜´ä›? ¯)>(4? ‰Åß K?4¨¿?¯{_®Ò–?—mÄ9çh–?ç%ÝÓk‰?¨þ£01¦?±ÕbÀN5?˜.ˆÍ›?ʀï&œ†?¦Î'ë¬?爫k¤ï?§h‹1?Y4_šz®2?dvx×?'wlÞt?¦íËI9æÉ?ï.Uü"n??—]m¡÷"ª?€ÈÀr$Kk?€HåÚ·\}?'Ðà8א_?'ªhè¯}ó?ïh/X!?ƒe(=«Æ?‡Qªu< £?v‡¢\Éø?'SÁ.y‰?yj9T…É?ìz4¾<ý?' °lÍfX?¦"hü	È?"›èøSB°?±%']U´?Œ-7#`_ðAGN3FGL J0307.3+4916@bAcÀB@TƒæÀ8ö"#—µÀ;KÒ®Že?Ù¶ˆ™'j
@ÕwQÆX@ÄÀ¿¿ãתˆ+µ¿Ú"ì¨y?¿åʖ;T¿ØË´¨'"nUNASNone?ï`«!½{?›J
Ÿä?Ú]­Oñê?<(€ÎÜ?–F»¾A®?˜ëÕHx=?ê|:ЭÏS?È-E›É'Y? ŒŸ'‰)+?¥™#?.Åä?Áëìܦxi?Ä¡ C?+?ì½ËZ0øñ?¢ØVC³§ð?¨ ÇÃõú?–ZfdHÒ?¬©–äHï?˜H%N<OÇ?ë™,D_3?¦Íßõ³Ö?•â¶Ml_ô?'<È+?½½ðL??¥nUt58?ï®5[Ï?~uL pg?jõá9/'e?f;rGŸ>³?{ƒŽVx¿P?yDŽ'EG?îI¢N°"ƒ?°ÏžVl³?ˆ™Oèb¹å?'m?3÷?¥?‡-[T?ªç!éBN?î˜dÊ*—?"uY´|?—ÚW€Ãª?‹HšÉ??•á¤êu?‡qÚþ?î»o;ïfÍ?‡³,VŽñº?€å;×
AÙ?m*ØI™XW? ½Kö.¸?…Úå"ͱYAGN3FGL J0308.4-2852@lÀ6âëÀMèÀh ÓÀ:Š7"D[À;õ½
·éç?Ѹg¡5+@
¹õ¯š@Kª@ýÁ¿çCr-nù¿æ&ÓØš¿ÚÀÇ2p¸¿ïÿNµxOûUNASNone?ï·×AgJß?;½n«œ`?^ßršÀ?nçáÑÅȵ?|\'ÆD ¯?‰µµœ!??ä"0Ú†?Ì×ÃðI?Ȕª¼¬™&?üGp¤OM?Å}Å[G?½½$Á³ò"?ì$½2¿´¥?¡ÓÍ҈ì?¬FcöüIˆ?""ÓP)?°¶änò)'?˜25'¹$?ä"ë›Þ²?¼mSž]?ÃÑ;‹5Aš?¸^4ÒeU)?Éß*4?³Ú¯Ôè{ß?ïXC,Ç֐?»{:åb?uXK'?žßîͧ ?fԂ&J?´"sŸÛ?ëQ˜A?¼S󇡟w?µJ†ap—Ê?³x<F¸õ?°,¹Bª•-?§(ÎÙ«þ,?íù!ŠFóã?'½,×àZ?¡§a˜Ì?3?‡Úé+clG?ƒÑ7>?†ž—wƒÚ?ë€jCsP?¦$Š"(*?´à9írÅÖ?¡Vhµ‰ø?®>e~OŠY?˜ÿvûÜAGN3FGL J0312.7-2222@j‹†DR?hÀL×Y‰ßsÀ:h©ÒÌÁÀ;µÙÅٔ?겸›VL@ ¯Õñ
Ê?ùÿ¤ÐÚ?îR'äɘ»¿Û¯ÈqÀ®ÿ?ÖáëxşÿÖÃò™Ì*¢UNASNone?ïօŠekŒ?qÕ¸½!X?QÌ®Ì^ r?PjM–Rg?pJR9×?on†˜¥pÅ?ïn'§.z?2ŸÓ8"?o`ýѾ'i?w'D3"ј?ŒƒËH"B?‰ãžT§=?íÔas¿??œ[r^ŜÓ?ðLµŽ?'e]N?¤1vSE+Á?'NFX*ö?ìî±è+3F?²ËF{¬¢?uÂñ"Õj?†9Ú9S?·.A£6Æÿ?²dB¾¤<¡?ïÞHÁÿƒ?mǞgÇ(
?MÎë«K?L'¾0H8?js
LSÒz?jB¶3`Ø?ïÉeŒvÆ[?v؆Ãíž?]¨ílN
¼?^}*eÆ7?sâþløëÕ?qÔú©?±?îûP²ŽÌÑ?Œ~÷ÉþûÄ?Žȝ°X?'4V"€º?'"…[ޝç?Ý0bÂn¯?ï&|Ê«?"R'E­Ì;?~"Vgɓ?zÁxYz¿?"ÖZà¹ME?U•ì	AGN3FGL J0312.7+2011@dP¿Ž`€À?›Gb• ŽÀ:$o±hÃ8À;—¨=¡K?¿ÛÃ5#Î;b@XšJïg?û_¿^Õ¿ïI;Ø?áßN¼sÒ¿ÌЊqˆƒr¿ÓÔÃáÁ¦~UNASNone?ïú&B¥ø?=ú¿˜s?7›u—Å÷?øA'£3?D€£¶Œ)?<0èûVÆ)?ï{â·Î@ž?Œb"Ìâ	?k/@jÂVR?tÃÎÌ®PT?Š;éØ(ÿ?‡O¯ÓˆKë?ï+µ¾tÍ?€½¨·*¹?':0ù€2¸?j1½ÎÀ_‡?'l/¿ez?xVýs?ïu7&ݺ[?‡Ä[d)Ë+?NͺˆGÉþ?NâÆÜb^÷?b­UUug?‡{#Ê¥ú'?ïü‰¢øàH?.×å¢îç?¨sw¥
–?øù£éµ3?7½ÙïÏà?,p>}î·?ïÔª¿[Ë?pPRkCX7?U#µ3^?QUÑ3´ñb?paÝRœ~'?k@%'`zí?ï'éêÈhî?iЁcø
?v)ŠSÄ?\»ÃNlŸ?€Að…¤@?aŸÔÉ~å?ïÛÆâýæ ?aæã&":?<R#nS=?.&>B?pWlaàœ?aJcOÇ^AGN3FGL J0322.5-3721@n¾"åÞÀLY@_k bÀ9õM–ÃüÀ;ÞGòù?å>k¤Ø€Ï@.:âT@™* :8?Øj*ÊȪm¿âÓ¶Gnj>¿åß5C}n¿é'l8YÛ
UNASNone?ïí'F˜?ˆ;ـÐ?€ËHÖò	Y?'ÈChDþ?uò¥Ê€ÿ?t׫
ž"?ío@afo?°äüàº
@?›+!^"ä?ž2o¸°Ç?«ykI Ƥ?¨¿ºN)‹?íŽe3"	À?›"vmYD¡?¦uEÍË%?•ñßÏà‡Ó? ¤fü3MÒ?Š¸jÍÐÄ-?çÜåדWê?³ŠÝ
©ô}?»_xÝ·W?£åoOÖóe?Âܬ5J+?°®‰{û_C?ïÚeƒ+\ê?˜)=I?goÊctL?˜f›ÀS?\UdÆáå?]yF93¡?ï!ÞƎ3#?˜4w'àQ?"uöšÝ+·?‰añ&?'‰+èZ)¿??H^Kai?îúh!—³?‹uµ7$œ|?"fþa¦Um?†‹Ÿóà=ì?ˆ—ýØW?wô.En?훡:f?™­t9Z6$?£'ïáV?†(ÎEìÊù?¢³àË::?"!zbÂxþAGN3FGL J0323.7-6038@qB¼£n/ÀGç4.ÛµžÀ:|#²Œ¯¦À;àÖìá?K¿ûð ;´·@j‰9Ðf@"È߂\¿åy3Ѥß¿ì¬\`ÂÒ<¿ DÏI'¿ïÿ·`²zðUNASNone?ïÞh"ève?zÓÔJt_?3Hû†üÏ?8ÿÈyþ¥z?o.[‡	$?z4ì"lȖ?b©Ô‹?ŠªDuÒ?iS²h'ž?u©žÞøª?‰†éøµ<?"!]ÕÁ ?íƒy-á?Ÿš}úi®"?¢Âãï\?®ibÙ¹Ñ?­4ëÊ1õ˜?˜þ²L"U?ï¶eqÌ?¦8rê°?&vsã–??^°po¹\?¸ŽSÈÞ?lâC'A?ïÉ+¶x^?­—¢ñ͆]?>Hç%dö?zyšíùå?y'5x*?¬‰PP0?ïֈg9—s?pSŽT0ú?TîAƒ,k«?TêT\؄?ox9g?h¦ù"|6™?îU"'Çé
?"×o…L?™0t:Z1?…Ó¡ü_Nª?œù‡CU?+öÄf#?ïér´ä×?`ÙȵVµ?	S^³Û?°afƒ4º?f(íH!?`­€j?W8AGN3FGL J0324.5-1315@hï?»×²ÀIÖf¡ÉÀ:R\±±¾TÀ;Ó&
UÄXÀ	rö퇭^@
†Nž)Ì@,è…Ç*¿âÁEiãì¿î¿æ¬¿3?kîb†£k׿ïÿ¹±3ŒUNASNone?›z´?¢ýN'9?Aßwф¾?FD'È8?Œ¶;.âé?R5¢'Ip?ï‡ü×47s?'pŽC¶I?hèûš¶I?€ÑX'¬gã?‡Æ‹tzÁ¶?ˆ,ÙïQ?ëè<¾2'^?¢m'Z=âY?ª‰iȅ:?"‡çª£Ø?³yQÙõ%ó?šæ4U[Ìæ?ïr¦Èù{?–憡<©?ÏF¼'–?1"H–Ü׍?'ž#{Œ»?–Ø Œõ=Ò?ïÂ[̦ٕ?_Î/ç?:u÷Vy?:ÿ±Ÿ8?}*ºU1Më?~~ঠÍ?ïך‡Äô«?‹Z. "ì?RdÎoéä·?Tè€03ÈÞ?o3µJ›?‰ézsßx?í©´jWQ?—Ûý¦»>{?¢6½"Äñ?‹âRyL?£.PJæ?Ñ®êÖÑr?ïæݾ»?lf×'T:>Ù÷ˆà"cg>øù=¨\ñ?iZYN?lYaöãAGN3FGL J0327.4+5828c@aÄí(Œç?øÝÈgã>(À9vG…À;ûXÑRn?ï0=÷(ã@Âg
€F6@•À8–¿ÙÑiüÀQâ¿å®üd¿ó ¿ì="ßEu¿æÿBpÆoUNASNone!?áOÿÌuÜH?ÍV4¹‰è»?ÄÓÇ	`É?ÀØ$''?Ó^–"¢wË?ËRBš%Òð?Í¢Üâ!Pe?Ïy\uªY¹?ÂÛ²òõÅ-?»¢/· G?ãà\
º:›?ÍÁÁSÐjD?æŒYv'­?²mè"Ÿ¯?»P´t!¡!?£àçT3¡?È&?ëä{P?®¨Aä72Ø?ق¸ålßZ?µ¦<hô²°?Ïc¢€ŒÇ?¼`ø—šªª?ÖËuÚL½?µ½§Ô}¡?çç˙y–Í?Ëazו0\?±.K«Óz?´¡RD¢D¯?Çɬ0ÚO?È%-
Kº`?ßíêÂ^½X?Ô.zwüw?¼`Æåé9¦?¶YÉ@*†t?Øùã"&ô>?ÐÝQš&‡S?쵪qX2?¤_½Žmü?ªŽYùµQö?•ýðz3ÊH?²3%°v|t?œP˜ª?å&õ'x•¾?ª˜¯°*%?ÃÏUñ¬³°?¥¹Ádûu?ǔÔpõX?¢W¹nXõ¦MIXED3FGL J0330.6+0437@fp¯%;ÀD]9–úƒÀ9º~¸lÃxÀ;'ØåßÃJ?ìJ	
šÈ@|Õ@8Õ@ä`RP/¿Ï¹2À`qŸ¿äÖƄDƒú¿Û[kP…ÿ^¿ïÿðH°{'UNASNone?èÿRzÌÿ?ÄÃê_¶Ž?"Õ+Û?Âq{J?²ßf(9@O?µY˜À´CG?éÏ-'èØû?¼WR}n?´'%VþI?°šŽ.–?½vlBôFc?±y¼žÒ?æ-¬¥?³òúíá3P?Én¥`]t?±PöáŸ÷ê?»¹ä—²Á?§­¶™öÿ?瀜٦5E?³Âqó–?¸ðS[§©?¬ŽxV•ó?Ņbë\¯Ù?­<)oÇ?ëá~û]®Ý?¾Ê•ûTt¡?µºÊùkr?¹¢ëŽ;‡?¦rzUb†S?¬¸þ"+?ìݧ$"u?°|ÚÓµ?©¤ îþt?¤ÁdF£ï?©é•Ðú=?Ÿð":³\?êÁë?¬oª
?¿#6!5k?¦ïé}É ?°L99hž¨? ¶/Tëåx?ìE•Ñû?›yÜy¥?°Þ"Áà¸ý?"lˆ5æcC?©é…WQÒY?'wÅ"MK§AGN3FGL J0332.4+4644@b¯a¦
EcÀª	EùßUÀ9®?uŒÀ;k|Ìy1?í[µ‹Ás@
c?aì@À}àU•´¿á±²-þÛ¿êŒtª7e¿æËirµT5¿æ»Kô
˜UNASNone?ç× ÿ®:?ÂÄ Øß÷ï?©Ìòèc'ç?«Øˆk<ó?Ê0\Ãi:›?ÁF[¾¸H?âfU<SÔ?ÑpŒÄb߸?¿ï¯àØÈ?º`Mûò?Ó7qï"%?Êù~¤©JÅ?èö—û^?­#ÚviÏä?µêúöóë3?ŸÖŸ)W?Á0L#4¯?¤ƒ"7L?áïùò
¾?´Äғ.r9?ÆÖ>÷ž?¶ %£i?Ñj üh¶?¯<*À!"?ìÇÊ,ðŠ'?³1ŸÕð#?˜uƒe?™õ]§µm?³¼R˚l?°€zç¤Tä?êO'ÏÐã2?Ç	\J-˕?­Y…^L‡/?°K—w{B´?¾Ö¦Ñv»Ú?Àe%`Y(ˆ?í—ßK:Í?™ñššG)å?¡¶¯Úò¬?Žªõÿ]?¤Ë[mÿŒ?o$‡Ù?é	³#,æ?¤kBb2÷?¿ô0hþq5?¢ócŒÜ?·¾6zô›?•ìD/†Š±AGN3FGL J0333.6+0233@fÆÝ/Ÿ¾ÀDwŽ`€sÀ:;à5_]^À;»*‰@†¿ðÏpˆ©1g@
+Ž
{"@'vŸït¿ÜÏ?ѯ¾'¿æ~øù?¿ÇÝ0r9¿èæßé<͙UNASNone?ïÛ6ƒ¹wI?o•cûb?97'¹ZûC?8òÂC¦b?pÑK«/ß8?mµÂ:ëÂë?ï_'1¦žÃ?Žãôº/Cî?pÞ¯iäÇ?v
I'hš/?ÂþIk?‰6ŸùF?î3ÈV<ð?'YŠhÒ0?'éàmŽYè?%m'kÄ?£ÙÓEŒÒ?'£'p?î‰Å§A³?™ˆÝÅԜ5?Løm`‹N?SícW'®?¦ïÃؘa?™MÌÑ$Vi?ïî S©íœ?^Ã=G*VV?0€ePå*Â?+Iö.]©?_Ÿ?
­ß?]ž==.Pú?ïÍÄ}Œ·x?qçPü…ÃÂ?Y¾¡ªûè?UðjVx?rܑ®Æ(ý?m	ŒÒ©6?îâo`?"*@ød?ƒ'm'9€ª?ulnã–?š){Z†Œ¶?""ŒÌi–?ïªàN÷u?sµ­"Tã–?:…Ô;.ì?4¢UJmƒR?"sÙaÙ@?sO"v{H'AGN3FGL J0340.4-2423@kQÃóà7ÀJÆ)ñkÀ:œ+Àx*´À;ð|_Ìï1?À¤7F,#@
'Ù@µ/ßì5¿årekÐĺ¿Ú0—–£ß²¿äÀ9EñÑ¿¿áð™#ì³UNASNone?ï¼¹à¯?'쯃JS´?GXí¾íY?Id²ÙDù?~Á"ìü©?'"Ù ¡žì?šç¶?ªpyãç]¬?‡i Pĝç?••±¾º¢? ¹®Ið]!?¢ÄÃtü"µ?î4W¶}ކ?'	ú½'i¡?'ý"'d3@?•©y{a?£;ºÑƒ³?šÄZñ?ëåO
•{
?¥çNÇýôÒ?ž'26îZ?•ÛÞÔ{D?¹4ûN¶u?¢Òø"^˜Ó?ïZþ¤hÞ?»=›²{E?Us›‹gÎÛ?"iTa¾ýO?"Hñ¾ý3û?ºÎ~3s?ï¤O8*?‹½Íwäàa?j~'yö?x""Gf^?€L­N̓"?'k‡Û|£?ï=k˜ª[^?×ZƨL?ƒ²òÎñ—–?qìÌÞsÊô?Œò'Næð?x_ù
=Be?îðMW̚£?…t#v#^.?†§zšàG|?sä/'†T>?–¢—·D¹é?€ÈÆJ•µAGN3FGL J0342.3+3148c@d
â'@·€À2a"D¿À92»K›	À;,äd™?íϣԅþ²@ôÑø/Ò@5F@V1e?ïã–>§×¿çA½¦ˆÉ¿ç*éy<;¿åGÅ	›‰UNASNone0?í-†Â7®©?µÏ\›4Äñ?«Ø©)þ'Ý?±8>ºG>?¡Nê³by?¥¥˜'4?êèʅ
µ?ÊÓNY‡äC?±Ñg•Gx?¼Ìfå+,B?¶íªp`?Á}1»Ü1?è_r'd¯é?±Z€f)?¼^"É óU?©£|)BÛ?ÀRìœÆ±?¤Âññ­)?Ô{h±Lò?¶nX}`!?ƃ³Úž­¼?¸ÝÛ³5?à!‹Tÿ®?½g¡'yÊû?îÓŸÙŠÜ?¥YÇSˆŠ ?'[A¹²Z?šLMõüýß?"4ÊPà\?›M2VÍÙ?ítËòm,?ÁøoV¾Âb?¢h|#
·?°£$cµÒ¢?¦¡Øcv?¶´í'4ã?ìѪŒÛñ?¢©@©ˆ?ªçԜO?™pѤU"?§ý'"–ë×?"=±®h}?âW
uFJŠ?²\{ËMQà?ÀõGJy"?¨nèX(?Ò×GoUMd?±ÒnÊ;Œ™MIXED3FGL J0342.8+1321@eƇçÀnÀ?÷\9¼º0À:z¦ª#T™À;¥ôæò?ä0ÈCiûá@
LØÑÞ?þ‹¾_K¿ò?¯&ˆÀXu7¿Ë
ùЈ¿á®ä^ä¼Ù¿ÞO•vk¹"UNASNone?ïÙ[R®p
?h¥æä8ç?L¡
º†3 ?I-çlY¦?o|jY;?eU³j—ú»?îÛ6'¦–‹?¥wÉP›—Ù?€Â-PL?†ókБ0?œ80"€x?¢¾g¥ÈÕ[?îƒm˜^Ü?Œ*Üvq?'¹~ÚH?~OÏxE?Ù9s'i'?ƒâiÝ5p?ë¦ÁT‹m?¦Š0<€0^? T¡#óòx?—æåÔe'?ºŸ¤Ë{éÛ?¢äÚÍ¥ìŒ?ïð¿Êþ
?W)#ëç¢?6câp9=ë?4í³îÌd?Xçq揨?T1ҙ.ª?ï¡IG¶fÉ?ŠÇ~PµF–?i"NM5Rö?nº4Wj1?Hšrºa*?†šÚ͛¹?ïaþ'7ÒT?tˆ~ô½?€ÂMsw…@?gâê!X­?†¾(Å'¤?iù¶®"I?î‹©Û?Šíºå
Š?'{ҋ'?~»£´?œ êFµe
?ƒ"QJUÒ°AGN3FGL J0348.1+4431@c!Ù©T"ÀD=F²lÀ:;ÔÂeÀ;n=)HÏ?ºŽ›t÷4@-}ns%@5G zô¾¿×¥Á'~iµ¿çÑÚ?üð+¿èduØÊ1¿ÔDRû$¤UNASNone?íšý~4R1?±híòdÌ?"'2lð¶d?™á^×Ü?¬çúO½?­œWÊ?ëN½~ak?Æ#MÕÿY?¡Ûº_éž?­7O]Çl¢?½	&34N«?Á*pÁß?ì5–²´r¹?¢$ k'eÇ?¦þïðÏq©?"Ùç¶ã ?²ÓÒrb¤ä?šÒV4Ñ)9?è<jè3ä?µŠw Å?šŸo¾Ì%?œ‹喵H?˺fgVë
?´Í¡ÕoŒ?ïF…Ò´»?™ÍL ?w—á#ï
?©V ç"?'YI<d?•ºYÏ÷?îsd¤w÷'?±v]±4a?ˆó²¸Ñ!®?–Kt²hH?¢ŒÉƒ?©zcñÓ(?'ìÙÞ?¦œˆø'Á?•½ü}Ô?‡I#I+#7?—óèß@܃?"Úؒ΅Q?í·íWºY¶?—Þ"Ñ	t'?"¥¼ˆI´?yð £zã?¯W»]ü™ö?–rZÑ·âAGN3FGL J0348.4+6039@aßî$5in@‰Ð~25À:2‰'
ÙÝÀ;± žÛù¿ÓLI¦@
^'í'úÇ?þ4A%9J?ïþ"¯OÖ¿ëÞðQJö¿×<•ì»Ö¿…8…âÀo•UNASNone?ïnQðk@?'ô }íÏM?9ü?e×6C?;–P‹Ì
?'ÍÐüÞíŸ?'ÎÍá}f'?ëîÔUú€?ÍèýûÀ?A:ëŠéX?˜19ãðb¦?Â0ÿ¸m«?ËîôêΠ?í
w[gk?¢¼iæï$ö?'a—"/¥–?'t,Cs%ö?³ßZîãù?¡—.!©Ý"?îJ9ºêTÑ? Ìo5Á"¸?B=žMLAA?P誛Aü?«mØçŠ? ÁÀ®u7©?ïÙ/‹€H²?vªÕ^ÊCc?,¡àtöu?+&8Ä,Ã?rƒ+:5Æä?v<˜$5&Æ?î¯òÄá¤~?º:b7¾Ä]?vZ2¦Èb¤?‰—ñSò?¢5^*‹M?·y`±;?î¼ðú9Ô?'`:‰[~?†}Á—-?~@¹t{‹??f•1ì?Ò-hj?ï¬ÚûÝ?wZ(·!žo?2yζ¡?2œ'^qFx?"5xª…(	?w,"m
ŽAGN3FGL J0351.0-2816@l,@N¤©ÀI:žË1ÂÀ:½4Ùü`8À<ßÇ{T4¿æÛL@
1S1€U¦@WL_ª	©?ëB³ÔáÌ¿ÜÎÊÕô
K¿ç-@µ‰˜¿Íp³G%ëUNASNone?ïԁ¨ûÑ?u
B¨‹ïÌ?Ih`Œãðü?GwI«½p?r'}wè­?s"¦©,¡?ï}÷¾#Lò?æB	|æ?h(<ö²¤°?vœDòæ?Šx:ßò;?Š±9½àÝ?î!$šÄ?"£^lÜr?–´V/øÆD?"–Ä_è^S?¢"":òÔ¥?Œ-ý:êô?ï	[Ǹ!*?—7,œS"á?U>''Õ4?\•X{È÷v?€žÞÃhw?–×¢"ð?ïîÚ2à?\V5OÉ?8ÇR'í,?5xGɕE|?]ôJÀP?YÌøˆš´?ïØHŸ"'?n›un6?R\2C?QÂnì#'?n 	7Ȭt?hÅü|$'-?ï%óO³?'%çW~øG?‰8ž'ñR?v‡½µ•ì?JšÌØ1ñ?watrñI¼?ïÙÒÔ î?mÜTyïõ?+Å«;¦}Ä?&l:~<¯%?r8ƛ\s¾?mS2kZì‰AGN3FGL J0351.4-3248@m"ßÎ1QÀIs,B»fÀ:eZJÏ1+À;õ¯OäCâ¿Úp6Úîµ@JÌõfžð@`g "I׿è%¯ó´Sj¿ç=‡ëlm¿æc¨]¤n¿ïÿê†úŽ/UNASNone?íGŒ4ðçM?¾?î¶\Q?jí)Ó©Ûê?vãмöâ?´ì5
q¸?½¶åfÃûº?ëéQ†k¥§?»9Ž½?§.E|z¾§?ªº˜³–?µQ­¥z?±_&8öW?é¤a\¢~?±eÁaØ?±c 6±`î?™)þ õ;?À¼êr‹I?°	á°ú?ézvkl4²?³l=*?²Énã…?©dPºí!7?À±–Æ*œ6?­ñËbS,?ëa;ÕÕES?Džha_¸Å?u{Hãc/?…ÐP®Ñá ?ÁÏ7¾»Åœ?Ç쎢ßW?îòSÓwòç? Z>âTM©?‰'M­¯f?j8'þL¢?"ì^¶ºSÞ?•''~Vð?ì
$½hoš?¤÷z¦]y?ªCŽ:¹æö?•"þc›üb?²uø;vµ?¢
l^¶t?î…j@CD¬?'¢¡lšï?Ö¬#ÓÒw?'Á'¼B¬q?ŸgaçeOF?Q£z‡ÊSAGN3FGL J0359.7+7649@` Âø7´¢@1ÐWÙÛ©À:¥ID°FÀ;þb°Ï@E¿ÜôP‰Û5›@ñvæ;^@Sù`(´ª¿í,#³Iª)?¨,ôÝ¿ä8B¿è‰¸Ÿˆ	éUNASNone?ïøéØm·?Eœ¢ødî?CV8doŒŠ?AéßÐõ ?8"@]µ­b?1ZÅN\ú©?ïZ"*¢@?–¡luëT?|ªs¢?|ÃÊâQÄ?‹"iÍ©4¥?"P8¸¿_ã?ï
vmÍA?‹)²"së?Ž'L?ÁŒ?"}Ç´'¡á?ŽÐ,ëªåE?{|ÑóŒY?ïiiY¼¬?"BÙÑe‹g?}c
›êñÂ?tÍ×7ÇD?†ô×{Ô?~«Ð9$*?ïýJ—do?+`"6¼Ü?)$
Ò?%3†i6ä?"2}Ÿ73¨?›X®]ÿ?ï̝ŸãŠ©?xœ9ˆç?bïáfò.Y?Z¬éÆ}b?p9?{
çó?t«–r¥ë^?ï‰hóÎ2A?~ž¡'»³?BˆËtà?y?.Î#€å?|ý[á)]?máÈÁ-´?ïãÌûh8?`Q¸?Tè†Dàn?HD0b+Qx?a¾Á‹Ãõ?[jˆÎJAGN3FGL J0401.0-5359@p'4'¾‹ÁÀG'.œË}AÀ:ÚºÊkÉ}À<:L,(}?âׁα¾@Ý"bô@ɑmä	¿ã8Ûn®¼õ¿è¤ÐÌX*0¿æŒVöq€?ÒPJ¹?YæUNASNone?ïŠå­À?‹D·¹ÿ?\Ýý^«€#?jî'*[\>?‰ªÔë¯Z?‰ÂL~#j•?ï\ÙÒ? yý[°¶ß?qó"ÊvÛz?Œ	"þ?Ïòñúƒ¿?• ÷~H§±?í*V
¬4?œ¦@q	X?Ÿ+%?!'?æÿ
#?­Å³{	?"×m9¿>o?î«ö>œY#?¢bßApB?rqɃ-§Ç?ŒhiÁ|Ç?¢òbáá+à? q&¾ú?ïØk‰ï`(?r®Ãòe'?M´,eÊ×à?[Á††6!d?pµxJ$?oº	G¾Ó?ïÈêØm?Y‹ÍÙ0@?aI
íØÐÜ?€q,~ÀO¾?sRªÇÐÍ?|[ö;3Ç?îï_ǙdÉ?‰®6¡·&?ŒÃ+aer?€áÂø—'¼?"²ƒs³*?•ZTë*å?ïÍ`Ã0¹(?znȕœ"+?XH>~‡Ð?k\1M³Ç?s=ŽÝÿ&H?sü-4,¸AGN3FGL J0402.7+2616@døP›ùÆ*À3"{՝VÀ9Ó÷Ò4ÛÀ;'‰¬¼Œ
?—½Iëêý@\ut cM@.Ðg¤T¿èU‹ûÝm¿él"©¼¿å'Ó¾¬¿ïþ[híxUNASNone?ïÉ{‡ñâ—?u².l>3?cpŽ©Â®Ö?eï…êì'?q‰ô©>a?nA"VX8?ì]Š±/Ÿ?¹†Á·Ó?¥(-[,÷Z?£õ¯"™?²ƒþ—Õ\?³Þæ®4D?í ´Žù"»?žƒXG2Ò?¨åص?'MúM¨CD?¥Þэ˜?'¨ˆ«Òژ?éºÞÊ?ªÉ)°ü­R?¬. 8"b?™ëQ³L?Âýó"éŠ?¦V½Nôö?ï县m`"?c¤æ=Þö,?V'èGÊ?Vr ‰®?^ÊX¾‡£?VõO€!t®?îâi›hëk?¡ÆËü¤H"?‰ë].ÿÿ?‰"e%ˆJž?–½D`Ûv¯?šÒÒ@U?îªÄÄb?ˆš°‰¹ì?™¿í;8WŽ?€‰¶Ä˜
ü?çz/îp'?w'Ã*ùY?î1OqŸU?Ž4%\Â	?'¼][(Y`?{"ÏÕ?3?£Œá'âB?‰­6Ä7tAGN3FGL J0412.0+0229@g³ÞÊl À@¬e"¯OÀ:
㎰1ŒÀ;'Á.32¿'-Q^·ÿ@V±Ÿõ©@0oß`ù¿ç	mý^¿àŸÁ¿ìšr
±¿Ë×2®uk3UNASNone?ïÐñ©>ìê?}^ýeͼ?pݲ˜Üî?yŠ¿;»ß?Z¥ã8ýI?^?‡cèÛí?ï)QÕW?‹ÈË."Æ"?iu xØ?tŒ½3¢?‰÷®˜q_ð?†¯ZŸS"ò?î^À6*MJ?'_ê~ìøš?—?-<y-?ˆt­,ò?œèËù¿«?‡ÈmY¯$Ä?îÕ挚?"- œ)6?_í~ݦoÞ?d·?¡¢+IÀúm?"ÒKR>U?ïŁû~w;?¤[°Ý†m?pà)Ý´O¢?›vŽ†þÒÒ?h½°­böY?m/}Öv?ïÕS]íhp?oÂo'r?T=Ýh¾?P»jÄ­æ ?pG
À½á×?j
à'û8|?ïP¶Ôgö´?€»|1€ã?…lÖáÜP?wHÈ{n]C?†esù×.ì?tåæšB|Í?ïÀ쵱Ž?o\DW%‰Z?AÛõÊ%e?<õ›N7?|
×Ä{?n,+cÒSAGN3FGL J0414.9-0840@i;0©7 ÀCMs\.ËÀ:4õIØqÀ;Ï$Ù¸¿æ{ÄА7@ÚAP'Ny@:³ɹȿåªñ)gFO¿å¼;÷k˚¿áû&'ÕŸ¿ïÿ½¶¥UNASNone?ï¾æ‹ î´?…ªüêã}?HJ䑓?ñ?Gà:CqF?}ƒ]¨áºâ?…6L¤:µÈ?ïƛ}¾?—#%±ÛÓÓ?{¨L^®.M?~*Ä­Æf?—ý…]­?"N¢œ¼b?í"»ùÑ5?Ÿuõƒ,ù;?¦Ýê(ÈÎ?"x³ÖO?¦öVK¿â?"5ȯsÚõ?îj…¢kÐ3?—ÆF¸Û…?w')5u0?wrÇâÉ«?¦e`¯|¶³?•?­ñP¡?ïíZ9:ü?eMwÑ g?79¨–ëݤ?3«KÅdY?_}#¬w•?dKŽå†»?ﴁ®ã¥#?z|yoæk?d¦»ö¦?`!õÛPS™?{w¥ºÏs??u¯ê…n»1?î®?±ê'?Šù¯oI
?˜8zô&©?€Îh'…?'/ÑcfU?Q¼)IL?寮Í{Hv?t×:ÍÒúm?VÊA"ëá?T]õ1ó&?ƒw"i±G?s±n—Î@}AGN3FGL J0415.7-4351@o#zcslßÀFý<£}šÀ9þ¥é34áÀ;ø½$¹í?Ûytß꥕@
T—'hÐ@݉ÿ󕹿àe¸Û[ä¿çŒÁ!¦v¿í.	öV'¿³9¼k—UNASNone?î2d­Ãa?´üX">˜?‹Ðcit?"?q)ïÚÇ?¥åœ\¯'Ü?³½ì¬?î὘/ò?°½z¿ŽËµ?'qŠS¤ñ?œ:¢0ß?š¼"<ÚÉ1?¥½oÌ;Ži?ëÃM·îÄC?§}J
K?¥I¥ÈH{?"Œà&/q?·@¿\e ]?¤Sìü–_?íVƒU›¤?°0n?.?'8Ã<–Ž?œšýX|?²eý¶;Ë9?¬›èö÷?ï*%Vëbÿ?´[ú¢
«?q-‡¬@$? ‰'SÓ}?–oó3è¤?²hXëêÏ`?ï¬dV¹¯?–0Hm
;Ö?j˜ÆÝ_ò?‡ÉHIJÚ?|Ä!|¿?‡æˆ_µr=?î[z 7Ëý?•aÇC–šÆ?'†¥Œ…Ï?'T™ŽÌ«ÿ?¡H«tËJ?'¾I_&b?ïxNMô]?‡"~CŒ?k¥Ò—þî?oŸÛt$Õû?…8wÑÙã?ƒ‡z¬C$AGN3FGL J0418.2+3412@dzxl"hÀ'ǟfb5À9ÿ9¶ÚóÀ;…vfŽªR?Æîê['Ê@
íyøêb	@úg–
H¿â:|l{íü¿ëÞ0Ss´G¿§¦¹—Úµj¿ïÿù½p¹QUNASNone?êûG>Wÿp?Éݪ	ÿ2P?%	TÆ?§pPœôù?ÂAâ"Ÿg?È<:OÔv?è1ۈ#"?Æ×	9˜/À?µ%»1Œ?µHò)#è?Ä¥´Há4'?À2ܺðE<?èF+)ò?°=«‡WÎ?¶ù{"‡!? ^gæÚoA?Ä9)Ršé?­\¾ãNE=?êÐèutÌ0?µþÔהCG?—cr֜?žþœ3Åç?ÁÙѼ­?´¯€MÒ£?íLˆÈw8Ø?ł¾½%Ëþ?Hð)‹N?ª¿"¡?±¸ÐÓY?Â÷ïŽ rD?ëíò˜ZÍ?¿:Cí¦È?ª­²‹p¡?°1M#?³@'<êH?²`åb¹ÁT?ë3FîßÐ?¨×µÓÉܧ?¯!²¤ ?™nM¾äQ°?¶Ôï~O&´?¤B¼¢	é?î0øçÚ?™Ïlý?"bœ¢¯?Šý1½"ÿ?£?0)"?':]V˨AGN3FGL J0419.1+6636@a±+Iº@'#póˆ"À8åbøÜ°À;e¤ëàŽ?ê§cۋpP@(ÛèH©<@~@Jª¿âÎð´f,¿áލf_A¿ã°ŠÕd)¿íþƒŽ¯UNASNone?Ò¹óD
~¡?ÇlÈùra?æÃX&?ǟöü‡`Ã?h`ÆÒ'y?'Á¡ò'?ˁé+­?ÄXVG#Cì?áò˜‡\ˆ?ƙ¯"ùŠ¬?̳´ß'2?ÃÙùtåI	?áå5À<Í?·â¦CoB7?Õ*ÌåÔä&?µx;£Í­¦?¼+kãü?¡©åÑß?ÖYê ‰|?¶çþíH|Í?Ý9EÏu§*?»Å6•é5ä?ÈÛBŒÓž´?°_PFº/®?à‹P}ñÈZ?Ë«
F:?ޝÕ"oß?ˉkª"3½?‰˜%Ñí±?ˆÇÏ?¯?Üa{eQ—?ÈÖÍ!‰,?ÙU6,?ÄÀ\1Y>?ÅÍ¬ü?¾ZmÊ2éŒ?è"UžÜ¾K?¯/Œ>Õ?ƖG¤›M?«	¡J…7Ì?¬q‰ä}•?"¹DÄP?åDKx=B?­§qƒú?ÎßÊ£‡?¬v<>Áÿ?¹~Ig­,V?ŸÕÄç&õuMIXED3FGL J0420.4+1448@f|Rç-¡#À87:G#«À9µy1DEªÀ;TÍè«P?êûˆnp@µÇ'`@î¿ÙtP¿âÄMA§?J¿îŸ<=?¿ï"¶|d´?äaU¬žÔUNASNone?ï/Þð:æ?£ƒÕø0?x]5Ÿýìi?q¾ªéVÕ?"ìԒœC?¢72¤Ë"?ï,È5
}í?¨Ù"A§%…?|S"€ø?•h¡
C~D?"R5ً	$? ‰¥`Æ@ ?ë¿e1CU&?¥]w"Ôñ?§;û"•?–ÒåÃþAñ?¶fØ­'ÚD? bÖ Ç?í'ÿ²}?µ1ùW‡_â?{³€'<Ìâ?—?=ÛíKÿ?µˈW'‡?´vÉZ'Î?À.G«?"ÚÄ, a£?h¹10ñÜÉ?w ¬jþ
è?‡bCâÊ'?äo<Ã?ﴒ^\?"‰Cé—fl?i'Òéu?†Ù¦hκ?xîkzÝj?…½ß ÄC,?íþüŒzn¨?›ù+g>?"CëÉ.‹?‰÷rá˗?¥îAPR3ò?—¡MI?ïŽñ©"Ó%?×Ù)Ù@™?W+:­YKÂ?rÝø
VK"?‰^.8ÁuR?‹º®ÎEYAGN3FGL J0420.4-6013@pò~|áœÀDäcÇOµÀ:—Ì9ÿÖÀ;åï3ÿáÍÀqãá'Tý@
š%ۆÎç?ý†Jßø"¼¿ìCÉ»A×]¿Ä|øƒßÈþ¿ÞM±Ôx蟿ÔkËCØUNASNone?ïìÕuÌÈ?X,ð}î?,/*¨J$í?!¾ò@1?ag˜_ó³©?WBpE=óë?òzE?†Ûe•%ٓ?d ¨*!ÚÐ?sœ!iòÍ?"ÊÙYWr?€žcA"ª4?îÈãÅHb?‡/²5¡ì\?†ëÈÓ}qï?oGr?˜ˆV?›m¢ôòÆ?ƒyø³SV?ïݹqÙ¿­?mߔžÔÐ>è°?.5M>úf°­iÇ?qîç¦XI?mÖu˜ž/?ï÷;¹r/¦?EÕÀI°?ÎÈrx^è?ÙæõP<?O@¦ÖÐ?DЛr·?ïÞJRð¤?j–F͟¨£?PEË0S|?PU¯˜)?i»—\ª‡?d‡%­÷e ?ïwßjqŽ?o‰Ô¹¬?ye€œkb?\—ÁmiÙ?…U|œ#ZÐ?g¾»¯ž‰³?ïù»#=X?A‹ÙT‰¶>µFQ ‰&ƒ>ÂJÂWˆ"?IÐ
39u?AˆWÞä}AGN3FGL J0420.6-3742@n	E¶ÃvÀF˜#πÜÀ9[x̚xÀ;£Š:?Ón±Ê¤@凖ŒÉÒ@®m@ .3¿å?Æ ¿ã>ÍI¼ä¿ç†ÍmËNa¿âäӏðµUNASNone?ï±64ߣ?KàÝn~?q}€,ŒÛ-?s|µKÎ?uçeHfó•?qæ+Ž"G?ïѦ°?ž(0ދ?yK!i™»?€>½vÞ<?™K=uiT&?™ŽbԗŽ«?î+8²›j¢?–"Þ§?Êp?—{HfDYV?‡6ÌM~—?¡ŽÐ¤Þ÷;?ÅùÉÛ?ì}"Æ?¢>/Ègè?'ŸqœeÖè?‡‡1,àÃ+?·«ƒ'‹?¡6œ'ÙÃé?ïì«zC?aT4RG–‡?P˜†ªÅA?S!&}ܑs?V[C³ä?UmˆH€N?ï·(8‹ë9?€¸HXûÄ?aRm;fæC?_¶è¿Þ†?{­<£DI?|Ánj+ðÜ?ï`B}~?xæSØlƒ?'ÀÁvædñ?pbtë?….Ÿ(8~-?iêÏX£ž@?ï$†ý,2…?'©uËh‡?x¡±G`"Ë?c)> -?•F´'Æe?€Çv}kFAGN3FGL J0421.6+1950@eýR½<6À4¿ÉGNÏÀ9œTŽ†@À;]¹û8ðâ?ãø­âb@Ðf{Š
@¥ã€B…Œ¿ÙæÒ1¿æ}ô}s{Ö¿âö@O6°'¿ì–­™*ÞÑUNASNone?ìS*ۇ?´Zë§ç?©o½ÍâhÄ?§¡ž¾û?®›†ô‰?¬Ö­ä?êäƒéPˆ?¿n
Âëf?°˜÷½y8I?ªÂô>¨G·?¸F¤#ª6ò?¸ÅÈ}œ^?é3#¡?­ÜÔO·€?Áx˜÷?¦fÆÏÛë'?´D_<#èU?}I
s²?å#ÀYÕg?­cÒx¸l{?¹ÍõZ¤U#?¡È lfmŽ?ΊëX9c?ª…{Zkî?î‰=ÞÝÆo?§ø#ì?•´K̇,°?¢ºŸ‰ÙÄ=?™#øTPin?™ÕÎߜ#?íöOØãäõ?­ÿ7s­Î?›S¸gN¾‹?•Ã}·žŽâ?¢ñ&A‰íg?¥ê»%—b?ì{µŽt?¢;	ÇM2Ã?³-.ÒÊi?ÜD¥…è?¡BU–Þžô?ŽÉûÖ…œ?ë$•®¾f?˜¡Ö,†–"?±‰b"
q?ÄMÿµÃ?µQô~}]?"t¾mä_AGN3FGL J0423.5+5442@bϕBC@åœÝøªÀ9ü*ˆjÀ:'Ýr6~A¿±-ä?GM"@§ÃÓÔÔ@™€D3¿ãº¥¹ëý¿ìî­…M¡¿Ñ8Áïñay¿ê\ôïøîUNASNone?âî°÷¦Œ"?Îkèú]‡M?ŒúÉ¿%?'ëÉ0Bån?Ù:ÇÃäç?Î_ìëŒf¼?çù7[Xc?ъy>
	†?›»}*^^–?ŸNHö."?ÐU¾£iQ?ÐIvÖöò:?ÝQïÉôM?ºHJòl™†?»À¥¨¼?¤aôՔ"?Û¾ëæÌ?ºY5ó¤I?æ@bv Mñ?Ãïʙ§í?m\¤Oø"?nOC˜ÞÄ(?ÓDÊE?ÃáaUÂE?åsc}¹ûJ?Î(ïW¼)'?'El Üß?›~Õ¼î/	?Óôâ:GNž?Íø$ЀÕ?ìóX lJñ?Ã(×úþ8€?‹þèGãû?"Þ²P
4?´åaîšmx?Àéþ²‰:ã?æ¼|JS`O?¶)dçÛýß?±°m"¹b? ÀŒZhl«?Ì5ØE4Ó?³Ä½ú@P?êÛgk*?²ƒŸÙM?w2&´Á³?hÎ:o™i>?ÃØ͘ñöI?²@œÉT[AGN3FGL J0425.8+5600@b¸"t¼j@d‰Ø[À9ƒ!
–ÁxÀ;
¤$7îÀþü¯ég7@=ïN×Ô@Çç^j¿çü(ˆÆsÓ¿éäÅ©Re¿åa9Uâ	Ë¿ÇýºDMÒUNASNone?ïG0½Pò¦?œ
í·œX?džémõ*?d3£—³‰/?"†'¿3Ÿ?›Å÷Ä
?íBX|eM¯?Ãj-Z×?Ÿi{:|1?‹`Ù`?³óEƒ–Ç?Âb'V1?ëŠ
‹QàÑ?ª»ñÇÓʵ?¥Í6f¿?—¼X‰¤œ?¸É£Oö™?¤`3Õ2Ì?ï4MŠªñä?'Œ¶3¯¬>ôÓJÂß&‹?¹q×~¦ö?™qψ3®?'Šá×GÔ?ïØ!€>ï?w::Ì¢5?O,Ë"?O
!õ|¯ã?p	¦˜ÂÆo?u—Ô6g^ù?ïL\0qP¿?²+t®'Ó½?h3	h›·6?'<nŽßœ?"nÃb™<?°'ëœP2?î}šX™?"Ý£™(®Á?'µ:™_á2?"ñSsÖK?ž—zjU ?0÷Hë9?ïÎÙãhÆ?kkd‡rÙ>Ðár\Ýr>Ðŵ±kÊ?xŽÖ<Ð$w?kišžŠmÏAGN3FGL J0426.3+3510@dœP	,ÏlÀ#P—ÈAîÀ9¿Îí8}À;.6Dÿä?ë+ܱ`#›@À;#°@èÏßüª`?ÄE¤—­¿èäKGbPh¿äE"‰£ñü¿ïÿô_
ÄUNASNone?Ö­Ö¤œ¤?ÎÊ÷ªÆè‡?È6gæC@r?ÈhËRp²'?Ý6ö	9Ã#?Ñpð›/?În—"Á#²?È3µuSz?Ø{²+>zÃ?ŒGwÛó?ØM
àód?ƺ²KŸÄ?à€¶Lýg?¶Ù‡­ISû?Í$ùÁní?±Kx{÷#6?Ðl®Ž§?´!ìЕ‡¦?Ï/h~Õ¯0?¯Ã€pÕ`?×_úºNx'?¸",·qõ?ÙQF¯×?µÝÔËJ ö?×ùŠ?ÑãàJê?Ã'6ö?ÅœT4	È?ގç³q˹?Ò¥@gŠd?Ý8.@kf<?Î!cÊL6?ÒSi¯_î?À{÷·Rp?ÐtÆUå9Ö?Ã<"*ãü?æVvžD#?±™W¯]š?Ä\T:{L?©ÆÜÛ©-?ÂIÑKGã*?ªo©''c?ÜH!æÉg?­QL–	*ò?ÔÎw 6Åÿ?®a;ÞlKG?ÍÒÍñÿ¦?§[E˜\úúMIXED3FGL J0427.9-6704@qr(õ\ÀCE±cºº|À9cGK,GÀ;Óêçj¿ÜùüP¸@
‹ÝT@¨`ÿŸ2
¿ãõ趧
_¿çt>!½ƒÈ¿åXbü"RÇ¿å\{&kUNASNone?í3÷g;^·?³'qOq¯?†¯2	(?…ø‡FÍó'?³žnÔ>É#?²xø'·ù?írºâWè?¾ùèõÞz?˜óüú[á?«ð´)/&É?¬Z`!Š?³Û|®uu'?ëT†«'y÷?©ö"6¯Á.?§#%>,?"ùCŠ?¹Ö9ɪ6?¤rìçŒ{?ëá»`,ª?³—.C*V?šVš–nÁÕ?—PÿO?À©¥ÀÄUÛ?±¼í/
¡¹?ï]¥Ÿƒ¶?—'—]O?iY«×"—Ç?pÅÖñ¹JJ?'15×þ.D?"x´ùo¸¸?ïLâŸÍ?©ƒz`}Ë?}ÿ€3/?"ö(ð÷ê×?ŽwÅÝt"?¢ µâb{Ä?ÂÓ5?h®í$?'Ôõ.û?ÔLwþŒ?›—w—fM?†"Ñ"m?îû]/æÖ?;eLY ¸?r3£ŒÝ??f«ñWí'?œe5Jð?Ž˜ ]H©"AGN3FGL J0429.8+3611c@d"ãû½{ À ނ/ðˆ"À9vygÊêÀ;õÊ?ìms†"
<@
¼¹"EŸ@üŸÀdµ¿ÕË룿çå#üg!Ö¿áÎ+uéU¿ïÿÖµdUNASNone8?Дœ®»h?ÈFZâ¾j?ÆuèYmZ?æÅÉoÂ}?â7¢aFõ?ÎÝìÔBü™?ÍT}q?ï?Æ+—'	[?כ–~²­?ÁÁ#XA,?Ùº*À•S[?ÅÕS•9žÃ?Ý'§ó¾B	?·#Ô³…"ã?ÏõP?™¯$?±"U€3?Òݯìtæe?·Äš´üÀ?Ó‹4ÑîË?²)^ŞŠc?Ѫ!Ïç$?¶¹SR2]è?ÛQRûG?µëp<X>é?ÚKZ$hU?Ά=«©‰?Äy)8ÕÖÙ?Á(­®hM?Ûx>kˀ?дýñ"?ÜSÊöfÈ?Ì!oåÚ?ҋP&¡?¿oñ»ªÌ®?Ñ åsy—?Ââäôh2?æ7AXÌ8?±ÁF""?ņug,¬S?¨nqiþ?Áœ…3}}Q?¨¡Òò,?Þ7víOØ?°ŵ	Y?ÒS+v??¬:ÃS?Ï#pùÎsÒ?§wR™°MIXED3FGL J0430.1-3103@lìÞÊl ÀED¤Ò²ÀÀ:°+Xs^œÀ<
Å󔷳?çß™3©a@LzNP?ÿ‰ÀGƒL?ïý-óáÂ0¿äéö[ïó¿Ë:B†M[¿í€.ž*UNASNone?ïƒô›ÎY?Š¡O+‡^?"#´c,?…0h ÒgÔ?u¾J>Ä·,?w´ëGÝN?ëb§-ð—ò?¸Ìra^?«ÝèW[ T?ª(¸Î‰?¶ûÒc¢I?®Ðzìv?êDµ1_?ªýB‡û<?½ÚjÔËÊ?¤›5"Ñ!µ?°ØR5-¿?œïLó[~l?ë	ïå·2?µA6JýšÄ?¬•"Å£Âû?¨ˆë,ð¹?¹eÀ®nXq?¯ZÞi…¿?ï˜øÓw'?‡"ið8×?€Ï¬Û…?'-aå[º•?sEøYÅW?q{ì[³½?íˆoû>?¯ãÓo@d%?£LÈF?¤ƒçÔkü?¤,8	Š,?y'%Œ?êÔ!áï?¨^;û?¼+"ÔU$?£æÖ
hHi?ªgÊʬ¬?œÓwæàW?î1…B[€?˜A`š
	?¢u|wØ{B?ZaÜz%?"äfâÜ/v?ŒI¬§AGN3FGL J0432.5+0539@g¿—$tSÀ;ZÀh ÓÀ9ŠDZ¢ãÅÀ;Y»JÄIq¿ípƪÚð¸@Pèà©£@ŽÝŸ'禿åëô¿íU
:ç׿×ÞÞY‰€"¿ã"+Ù-ÆUNASNone?ïïŵ"Ùk?aâMVÝ©?(X«äcåà?$-Ԑ¼üš?]iÛåfõ?a^@¹\…?ïodq™ P?ìV¬"[?p+XËÿ?wíӄVN\?Œ7(îÞ0?Š¾ÑԈ(?î	בÌ?—¡BöÃÂí?Žª>¯ ?{?[˯{?§·÷Dý?"¸ÅW-P€?î;´·^?›Þòã8©R?A¸.	@	?A/ÚØS?¯µcÿ¢Åº?›ÄZòƯÈ?ïøüDdU?FªãDn?I!OÎ3Ž?6±à•'œ?H&¿x@b?E=~ÍEÿÈ?ïÐ{êq?q™"—)á?Wä¿('¤í?R™n'ýr?qÈÛv\ƒ?lîÉ7ž'J?ïOñ¦1=Ì?€Ü€Îalk?zŽ®ÿv‰?d©%"°Ke?Ž¼Œ–Y{Ð?~Ÿ7N‡Ø?ï…S¬O~Ã?wD@Ðko?1÷Â?#ÙNÐ+Í?Ž\–EZ?wíÐEܽAGN3FGL J0434.3-1411c@jWŒ½D¦ÀB[hœ¡‹ÖÀ9ñƒ 3ÏÀ;œ£©½Ô¿é •ìÄm@ü'ã@Íÿ|wu¿ÛÀ)˜œ2¿çÚý<´ÄÌ¿ï"ÿž'À?áv×fJUNASNone!?ïî%Ÿ'Ï?b÷ìäƒóv?J›J¶~'?NU¬"ÓÛ?Vhfø ?^dD•¶¬?ï'C6‹'U?OpÍêÑg?fœ¸FPÆë?y[0H¹T?†RÂg?‡yA_pÓÓ?î"Dö ¥‰?–h­+R?•'v«&5©?‡˜*h:OR?£uHbŒ–?'Vh­Ã'?ï¨BÓ¨øÌ?‰AЈWͨ?%à`k?'9výÂÕ±?…ÍDÒþü0?‰:»ÞUê?ïø}÷ku´?P('ú›?0´h8Gß?4Qƒ2AçŠ?E­â°a3?IÚ>$²ª}?ïÛbû‰	?ooÓÿœYõ?RlqBÛ?V7»@"þß?kföÓâ7ê?f¾%ºƒ¯Ý?ï2fµtI1?‡;­éÎj?ƒò$÷‰Ô?x†–¨:«©?t-¾é?ƒ&2$݈p?ïõ¬øF"N?VUô%zö>ÛûÒ¿÷>î&å9×OÄ?TŠø˜Ï?VIdˆÚ°AGN3FGL J0437.7-7330@qá[À6ãÀA˜À½ÊÑJÀ:6`áÂ'WÀ;Ô}Qœ?Ú:¿ö@ý
WFã¿@Êß^Iâ¿ç4ãöERV¿éæ—S™/<¿¦·äüLð¿àÓ´[x	UNASNone?ïùÞ[s è?AïzU5¦ ? ˆCøU6?Yí½ñ}?Eò—DÆ?AR¦sŠ?ïi!À'x?áÂ_Ññ?m÷'÷ՖJ?uœ¾U¨`?Ž"Rʯ—?ˆŸõ¬©'?ï@aˆÊÙ?ƒ…
®^?ôÏAœµ?mr$a—¤?•}Œ*—ć?¯Œ'ýu›?îö[d?•BfS"?Wã÷?ÍÚn?du%¬o¾?Ÿ¾žÒ6ÅÄ?"«"hØ?ïüäÊý ?-Ò5í
0?"oþß?E,Ö÷Ô?5#8/ÎW?+AkMŠ†.?ïÏ0>D?qҙ›ï¨?Xmp%–åM?SÔ¬\\å?rañk`Î?m>ÿ[øžÂ?ï–^0Œå¬?lrm¨së?sKÓu*÷í?_FÑE?€ÂŠ+Ð÷?ee¤DÑiâ?ïDZùütŸ?nS°eß©?Wƒœ'Ü+£?Q(B!ºô?vFùËÕv?i¹‡¿
/AGN3FGL J0447.1-2540@l3E¡ÊÀƒÀBØò{²þÅÀ9û=5´ÃÀ;ÓFóÚWпâɽé…Q@
>쯖0.@ÅàŽ6¿å<Ó@Àu¸¿æTþ&¶øû¿ç;M—ý& ¿è
&S?±àUNASNone?îjlÇmV4?°Ðp/èÐä?uø¨:v¿?€µAï"]?¦¶Ts÷Rð?¯R›?î¨Ä—¨*?¨H|"hÊ??…ª]PD?'øØ"Ô0è? /Køõ÷H?¢Q9F‡HÀ?ìÔZñÏKé?¢
vI À?ŸÓúY°?Šzíú{?±hg2M?œFDJä~?íÀ¨¸W?¢©í!qŽ?ŠEÔ(>k?ƒæ°–:àk?´KÑAû?¡ioAl·?ïgBr1?¤w¹²Ú+‡?eb`Ðÿ?w­òجT?t¥uCCº?¢²Z¤Ÿ?ï Vömh?‹gr±Ì‹÷?jš€—½'ò?vcÚP\#˜?C¢.¥D?ƒ'YªZwì?ï'A&TÂ?'î}M¬?‰pHÿÔ?t6	dø9"?"Cµz™Ñ?y¤ä¢í°f?ïcLjÑj?€	gnaz?epqÊûê?Xm_¤·L5?Ù«¯Bd?~l!—с¶AGN3FGL J0451.6+7231@aXÓZ…‡"@1‹Ø¾r–öÀ:F–À¡E`À;Օsš+?æ"+de@
فÞç×j@5.?Ù^Ö¿ê7þ¥ü˜0¿å/–¼¿Þ0‹"iAô¿ê'/îÀ_UNASNone?ïÕFE´•?sƒáIÒ?jø¸L?m¬':í??_'(?\Îzaª?í@ô"7t?³òQ¿mò*?§eWÇ`ý?¡ÿúúòø?§¦™¡'É?®	øvO»Ë?íž{ðU,?¡ì$?¡ôò7˜Ý,?ŽØ½ñ½?­¡&Ñl?™í»÷ëÉ?ë"r–Óõ?°‡gD¶'?´ñ.–kfÖ?©…|ðèô?±û<±="–?¡›‡]ìj-?ïî®ïõ¤e?\-¶{5ƒ*?T՘'‡Ä?Tð"eþ0 ?K™zÑ`ˆ?F°2eGR8?ïÂÿª«Ì?™Qïå?Z??Ž<šA§×?"¨_°Ù|?Ž¥Éþ'@?'ÞÀ•0ÿ&?îì¸ôcû¹?‹S+1öÊ?äbKñ?è°JHj?'v°,ûX?ô§<["B?îríÕ¨`?"~"°€Î¸?§?ø,<˜?ËØþ`"?¦ä£½ª?wW‹ëMÇAGN3FGL J0451.7+5722@bã©æî·@ £›ˆ‡"ŸÀ9¸ÀÂÓNÇÀ;n:©I:?ÜRVMƒZW@
¿Ñ2œ_@䜿¾ÇQ¿ïµoŸf&?ÐXÞ_闿ÕÚ`:Ê£Ÿ¿àèaÓ¯•UNASNone?ïk.Å÷W?'ìA\@ȝ?"4(¿O€X?‹'{Æ}…ð?˕¹ëí?†[~¨gíÄ?épLŠ¶ì€?Çlj	ÿ]?±Ù¯·§Çf?³ø[dãV?ÁQõøâvÐ?Â"J"Þ*?ìYGÍ|©?¥rB¯Ö['?¤ô±É4h?'ãE q?µ"ÜÞ±´j?¡`Y ÉþU?çí@¿Û8?ºWãßÁy»?À".Äõ¤?³MÞÑ7k?À(Î;÷?´,Ï!jþ?ﺭÉãt•?ƒÕ€Œl´X?r=ÝÂNªÄ?{ôðô×9?pk=G'–¦?s÷×JÕh?íÚÞÿ¦?¶/pc/ô;?—Ò®õ1¬? ƒéŠñÖµ?¦h¸ª²œ?®Úºân¾‡?î®"™nj?·;eè¯Z?'|@t7ªÿ?"ú¿?˜ÃŒü
#±?"ýZK@"?ì³úuý]8?¡'mÇ ì^?¯Ù£j•Úy?–¾2rqv5?¤æµ5"R?–;i†®AGN3FGL J0456.2-6924@q‹öy|ÄÀA¤6~ANÀ9fÁæ¯ÍÀ;ŠCV–åŠ?ôUü¬
‹@!ÓÛߺ:@vQØ7?Í6;9¥¾¿é¢<²I$¿å`î¦L–˜¿áB#hºÔ}UNASNone?íâ¥ZSCÛ?©"çÎä\¿?¢~Þs¼…ð?£€P™áÃ?ž­—ÏÖF½?šØzoŽ?풿ù]W'?¸'ªhï?–ô€'Õ'?¨SóýP=Ô?«YÀUdU?±žÀÜ|ãÃ?é½ãüFë?­qR¦±Ç?½= 
jæm?¥'{ƒ‰*ï?´Ó@ñr"? ÙGô$Cp?æÁiŸßb?¸ÉS›‰?¸±[âÔËõ?±¥©:ìýÿ?Ë(Li(ý>?µ³'*?ï?W{3tn?">Û?Ž©ñÁÓé?Ž
"|¥ø5?'wLچ?}Cštåùý?ïgÕYì¹?¥ÜNàbÖº?†ØE)i?—ÞþC^Ç?"$™:ĺ?›à¬Q@à?ìî!.+•
?¢'Ÿ¸.¿?¯m_q-(}?œ³"øø±?¡°©…Ѻ?'`%']P˜?ì(Ý·W?¥µÓ ?°x X¨ø?fýüIÛú?¬'
ò!p?š‹qr:{AGN3FGL J0502.6+1759@fö©ûçl‹À,~$5inYÀ9¼R¯Ð<ÄÀ;@½½eP½¿øŠÖ/¢!@˜‰°B}~@TZ 4"[¿àɪÄöOä¿í¢ý††Ÿõ¿æb"9éŽW?ÒZðiÃUNASNone?ïjv{K??šÓkîz?Q'þ+1ç?USÇ:¯-ö?'§0+c?š"PJv4?ïFi_ ?'¬C÷Bð?nº<f_Ü?y&°ý—?ˆÖ¡x:m?Hëù…?ì'zvÇ:D?¢gëîó_«?ž'Ûöe–k?——'¬‹&?³ÇµLš»Â?Ÿ²Ÿü"xŽ?ïZtú4²?'½®ã>ø(œ(b,´?
`—æ»XÅ?"«V"16?'ÈÈcå
?ïÁRY$o²?ˆ]ËV7í?<çñ¾	Q?A˜ցÝg?}ˆaò9?‡±ð,í?ïÔÝ*<?tS÷EÀ­E?VwMlpT?W¸ÐH.ÑO?oç?_&"6?ph>üiÆa?îkaÞtó{?˜¾ùF¬?ˆÓ¹«%ëÉ?|à¼ñx?£ó¯Ÿb?—ù3e»¤9?ïãg¶r˜N?b¥U9˜R>Òö'Z´>ÙáÀ{ï´Å?lŽÎt¢«D?b£óýE¸AGN3FGL J0506.3-0357@i+IºÀ9{úLaØÀ:©­
åÀ;vj!
?ññüÌï²U@
sà!"M¥@W=ÿjþ?ïøñ¥8"¿â4z/"bë¿ã$–-º‰¿îL‹Ç§|UNASNone?á)Ý!êǛ?Éч$T¦©?ز4Ç>!?ÉÂCÃ	´?³èCՒ¥&?³ž‡E'S5?³À©ÄX6?¸5sX¬l?æÐ|…Ƚ…?Åù¨‰1Ӟ?Ë3­"ÖÄÑ?ÁÄT‡…‰±?Ùm³³\t†?µÚ5åƒì£?Ú®7ì5À?µ´G+‹êœ?ÇÈ*"Héö?¯^ہ#4?·­X¢GVð?¦…uåÔ=?å1•V?Á$#)*?Ïa•q@ßï?¼3ö҄ǥ?à§ÂɋI?ÊԀJh?Ú9îY –t?Éq–ÝÉì•?±Ú0Iµ/ì?­G_¬a=?È.E<?ÁÜÜåHĕ?äl°@ò?Å?FÐ&§?Ç|
E0ê6?ºÀªâc¯I?ã†E8G6?²"zU?Ò9MÓaUI?¯å5áO2?ºèžò@q,?£uØ]ø?ÌFH󨝇?¬©|S¢9\?ã0Ì#+€?·p%Da?Æö†~"´z?¯XµWHõMIXED3FGL J0506.9+0321@h¦$žDúÀ5_â'@·€À:Œý­?hÌÀ;»*VëŸ ¿ùkm´3@Eþw?üމ€Fâ=?ÐaÇnÅ?¸*Ùô,׿ßAׁ[µ¿Ý&ÇojÆóUNASNone?ïçKÿw?_w,s?Aî~õŠó'?Añþƒvg?d8`Íå?ZöŽ
ˆ¢{?ïGò‰X7?¡ÇôhûŸ§?vH´f.÷$?™~"DB?'o€ÜØ_\?–ßA§;Ùû?î†>aÔJ3?Œ]f¨úŒX?ãš¥¥nú?zHœ7îص?ŸFfm|˜?…¸~ZO·
?îûc¼?"8×Â1-î?Sà•[cTk?YIÐy™ºÍ?ŸNUÎh®??"Þø»–ƒ5?ïó@Kõvå?aóòÔãc?2*}
ôœ3?=ZšjÇ?TôÈNðÌY?]ÓÊ?›JÆ?ïÊ$ff¼M?w†á&ê.@?Zm3©·‰?U²±[5ê?tI±yˆÕ?tŠ›¯ˆk6?ï\øíÑì?xÌ܀3Ã?û¸´›4p?j[ÍM´î?ˆÃèfuË?sRêEM?ïÂ!е9³?pe›|©?$m8õ-?"ô˜÷¶
D?~K«l=N?pCcüŠAGN3FGL J0507.5-0906@j)ˆe"¯OÀ;0÷Do›™À:w©"ÉÀ;¹/š!~Ö?2ÏO§°k@S[žnH@ÀÍÆ¿à£ûiº¦¿çˆ¶xU.ä¿åÁȅÑvç¿Ø¹û{ƒPyUNASNone?ïœZgT£?¡l‡??T½"Ûžƒ-?V¹ý²àÌæ?†fxÓýøÒ?¡YV̐Î?ï&㶕 2?žOÀUǽ?yÁÐWa^ì?'i1âù'?"³?™µ¼n?íîy¹¢E?–ç†êóÜå?—‹º ßºä?"Õ§kÛ?¥R'AbIA?¯ä]û½?íãj'V@?š'€Éã?tPœ¥b?sL²»÷ü?¯DõÓVSÊ?™¼ëQsðP?ï㤌‰2;?Š²jé?8CófÀÝ?9=…†Õq¥?iXjòá:?‰õ⹫ÚO?ï¾ËAÝE?}}º7Ã>š?ak¤·,™?b?p¯Ãq?x©<ò2?xÖ«ƒ^V?ïC/}¾i?>þœîWË?ƒÚCÍ+Ö?p5¹Œû?‹^ðP_"ä?vµ·¸ÌŽ?êf)™?vaŒc°f€?]4["4?P"ºqáZØ?‡óU:"&?tÅTÀÇAGN3FGL J0512.0-3737@n0mÚÎîÀAˆƒ¡	ÐcÀ:¦í_‹ÎÀ;æ»:Ôe?Ér¤|‰Ð@
u>mÎå@™Kãö	?ïÚÙÔ¶êÒ¿ê+ýw˜œ¿æ
W	.Û¿×L…ϸ9˜UNASNone?ï"ÆcÚ£ƒ?òwÝÁÝ?F'úòõýÍ?F ±£>©?eGIÄõ?…ËêˆY?ï)kq›¬L?¡LFëÑê?u^É"ºP?'¼™íµ!K?•zߊ¸¬å?œüàkÔZ?í¥e¶™…?™øLʌjW?—Í%ØÄ·1?‡ 	SÉ}M?©ÃX%?"íôanã?ìŸùb,?¯vÌɞye?"lÿ»?9?†3̊*è?¸§Oñ¢?®¿
"Õ?ïÍ¥>,OX?¦'KsD?G=ñlæþD?'DõÖÅïÅ?vE¢Ï2å©?¡µ¢A?ï¾ùÓ›Q?€¢Z¾?`F–œùó9?cìçàQ¡w?x_íÚCAñ?{·áa]W?ï¸CRæ?…Ú~p†@p?ˆœODú?vp*ÜÇÎ?'úëgCem?bNq¯ ?ïY¾æbӒ?ˆAo?k¾¡b
?dà#òp›Ú?'dëo­Àv?†l'_YE°AGN3FGL J0516.6+1012@hû¼¾bÀ/v(í_ŒÀ:cŒT6¸úÀ;yÇg2>A¿ÒÚ#ޒ®@Àà"ÍR?ÿþî_ċ¶¿ê…³tG`οâÔ¤::¿Û¬³Ì9˜Â¿À4?¤ÓUNASNone?ïï4'é2D?WÝ,fFx8?2³f7"»?/IäœÌW¥?]o$9i?V#wãÃ2?ïVüÍ¡£?—9¶gØÝ?t8ϖ_	?'ç&S÷"ù?¯"nä?'ãõñ#è>?Ð3?ŠÝN'Í'Þ?‹
UjJ	?t«)aìºÄ?ŸW!l9Ω?†lÐÜӊi?î~QŠ{?™†Ê@Ô?Hžh9ü"ç?Sªj4†H?§¼AEaâ]?™mچÆC¡?ï÷U†1?Gˆ1þ¬?$ 
Q'á!?ٚb>b?M¡å
Û?Dû9Ž±U?ïËGSюS?wRI4
»?[å£@3?]I˜J0Ë?s•Ü©™Uú?rCâ¡ØÿÌ?ïd³"•É€?u#,-oÓ?|û3lZót?dÇR1I§Õ?ˆUe+?o÷Ӟ똋?ï¥÷\²!j?sžÝí
?='Ëݔ'?8ðQ™?…•'r	½?sYѹåÏ0AGN3FGL J0517.1+2628c@fSµIùHVÀvvþdŽÀ93PdŒÀ;}#AM¨?އµËYÓ@@ó#x«
@=ô|ô¿âØ(š L3¿çŠK}#cª¿â‡ê©›^/¿ïÿòh´UNASNone%?Ü	ÎÊAÆä?ÐÑíÇÝéo? YOžñË?§èäÓ¦F*?àõƒ ðQ?ѪÞ̏ÌM?Û>õ`a6?Êó
ü)Ô?ÌX1k8?¼3›Öé8ò?֔ñê­Ø?Åîå´zF?á­,f~x?ºêX'­ ?ÀA
dRÌ?¥ÓÁ|šW?ԅ-.Ùª?¹'zƒ©Ã2?ÛÀÜʵŠ?µ»Ð\®"™?жØ*	O?°vI@¥\|?Ù÷¶
e?¶bM—ˆ?á½P¥ßÎ?ÑÉDCÉ$ï?–ñ½V"	­?›¹ÚáöE:?ÛBßEØ?Òm8è~Ú?æ:È﮵F?Ç–ÐÖ5›?À½‡yJ^?³j›Aü?Ç	¹Ëà‹?¿mTN-Vó?çD홏Í?²ëÙWt±?¶ïÊl|(?Ÿ&ÔÛ-'?Çx^㇛¸?°²Ç§+Ïþ?åe v駊?­}‡­BtÃ?¼#¤¸? d¢êò?Ì[ì\V{?©Ÿ©©MIXED3FGL J0523.3-2528@l†wFˆzÀ=ӌ†‹ŸÜÀ8£¼:®Q¸À;iÉü7ôc?ðî[Ý÷A•@R$óÅ@;ÿûù5¿â‡¡1h'Ë¿àq•¥ ê¿áUôúâ¿î²"ãøõUNASNone?؋ѽÕì?ÉW)½=¸?᠎cc/X?ÊÝ>Ž?°ÌEíŽÓ?¨†qR5~}?ºˆ¢÷U%?¾51
öv?å79ÖC Å?Èêƒ6UÒo?ÍßÕwÒ[?‰"i~?Üp"Ÿ3®Ñ?¶³¥ÊA'¢?ÙñµT`)‹?µ ҄äÚ?Ã<PØOH?§ÆÿkK ¼?Òt©',ŠD?·ÒwªÉ|?ÞýýŽXa?À^t_Mmq?ͱ¾ö·?´þeÆå?à#S(?˳0ãà?Ý!p1Z.ä?ÊÝ«Še|º?¤Ãñ¶4\?œð•¾h'?ǂÉ*xF?ÄoŒ]¾D?äpónæ×T?ɁsKëÖ?ƹiì\¬?·ÿLO.©?åsñûk­?².åSùF?Ð]ciB?®ú³µ1w?¶ÒÊ®2°?Ÿ!Þ"êΆ?á³»ô[?²ÆxµHv¼?ԍ+vH%?³"ôɳ-?À¹A¢B?¤êEìcåMIXED3FGL J0523.7+3328@e´×
=p¤¿÷"'àÙìÀ9;þ®Ç(À;#Ððx?ÁÛøCžu@
E¤—yƒÐ@b †ˆE¿äŒKÑaæ¿éè¸
"'r¿ë3R¼ ¾M¿â"3í~"QUNASNone?æú
þ5Ðq?Å$·´%¥Æ?¨]±Uç?¥õèÊ?Îü™÷–?ÃнOßÄÕ?Å+L]É?ÈÝ-&©¸?À{՝Uç?º%†aÙcß?æ–_w8F?ÊÂË6t±-?çïoì¡ÿ?°ˆ–Rl}e?²vƒœB›z?œ£EBi?Ǹq‡=?¬%!û>?âßÏ]ö«?¸Oºø­Þò?±ÁseBô?¨Ïï±ç	?րPÅÔ­?·· NÙEÆ?í!]ãŠÿM?´]	Õȝ3?~ߦt?ú&ec?³5?²i§ö×÷É?Óyïr?Ñk
÷fÿ?»Ý—qŽ¡?³Kêä¢Çå?âÇÊ&-"?Є‡9p?ìù«bü‹?ž¿3¦…,?¡8Î_–_ö?ŒÒ‡#nq?¯,I]ð`?—@n綍?ꥰ݋"?£É)½ß6@?›b†&Ì?†ýpGŠ?Áÿ¬y\r?¢¤{jœvMIXED3FGL J0524.4+2839@f7…ðoiDÀ.çğסÀ9SS@ï´XÀ;5ÛNoϜ¿ñš%ȼqá@ÌwSH§d@þ[`m~¿ä ñðÞ¿à(çY.ß*¿ÝC—ñ	¿àø®Ž.'¡UNASNone?ï\lsàfK?xóÿš?góˆôô?b×S†3d?'t‰»ö©?ŒÞfÌ>'É?í°²˜w?ºå€ôm`è?ŠÀ't`i?8â`#2?´wê,M½?¸ÄôxÇÄ?íÛE/[?™²uB(AÞ?•Fw¡ã?'Õû‡8Ü?§¬@/-¿?"ÃÑðZíù?î>ÓÛ š?"ŠÅšÃ¸?F/v§uïo?C甜›¤I?«ºæ	è??"iÖЊ0@?ïÐô]E¼‰? ,ý`©¾?P\¹e*õ©?IäjÝøMï?sn¢ë<ýt? *áwv%™?ï¤ë‡M?¡Bʓ­3?u_ő¥?vÓNÜ[
?˜£ŠÑX6s?ž°çDY?ïI/på¸?¬"™@Ñ?œ…_ºu"?mauSOÇ?Œž¤'¾V?{³ øùɁ?ï~²0¥v?thh;Ù?/
Ô»?$GØÔЉ?¿"?t>¸
߬AGN3FGL J0524.5-6937@q"Ë]ÌcñÀ@jq¼Û¾À:VýŸÓo~À;šFfޏ?Öà•©Ay¿@Âԏ‡?ú"YwI8?ïíNc œê¿Ýwúã`¿à(¨dQ}?Ì@´Ê'M	UNASNone?ïÜ›:r\?i;t‹õA?Fv.çC*]?DQ_ÎÔÕv?nCØÐÕn?gUùÙå¬õ?ïvñâc–?'6cEGþ?jŽ~©Å^?u4țzo?‹Öãï+±?hƒ+€ý»?îˆ![3FB?Œ¸¢+5#S?ag&G?}ö‡¡k•e?žšm{™Ùy?…ï# Üè{?í–ïžf‹?¨âºëEÀ?fßåݯ¾?w‡•öúÛA?²'ƒÞÏâ4?¨¥JL¶YF?ïó'úÓ?LjٚáÐ?1 {‰‹]?-ů_q/8?T"íªŠO?H›Ü¢Ö?ïÑøÛo?so¾3>â?V1ߙ(ÀŸ?UQwˆwT?qw|¤´‰?o·‰iÙ·?ïQaIF?~E¡èýè?,÷ ߦË?q¤#±m'?Šz¶;;Ü?v|CtØDÔ?yãyj?ƒ£HðÌÁ?R½;§!tË?["Þڕ-?Œü:ŠÜ?'Þ-¢Æƒ#AGN3FGL J0525.2-6614@qD¾aÏþ°À@¥ÌBcQßÀ:ëíúCþÀ;¤ß³Y^@ÀÊJHùn@ ]-X@Ý<à†(?ïóšÑýä¿ß(l\ìâc¿ãѾÓS¾]¿Óâ'–¶ªUNASNone?ï÷.Þö×?FóÖ¾ø¬?1©P§Õu?+Áo _?J|®­šS0?BÞ¿6"@?ï'aeÝ?ˆ6ЋC ®?f)VW#ú?tð]@?†bŽ
‹?'\–E\š?îƖº—0?‹fYýי ?‹K\¦Y?}Uˆž¥Â$?˜gƒÙT?"¢Ä³:k?ï|ÚL£Wð?ŒeŒô0@?´9wº§?$ܓD]y?P.ªù˜?ŒWÜ"d¶?ïû"®6ùU?69gÀÃ5¥?!s‹ÓwÃ?*tí´>?:¨ÇIeÃF?2%א'<-?ïÚï7/í?kxDîE:@?QêÀ¶
¢'?Pew@QŸ?lh8"i?eô½?ZÅ´?ïmk;?úŸ?}µá¿FS+?~çÎI¾SÒ?q6{FÝ1?…1JÓZH?w€M&Ö+ç?ïè(X
Þ?b,Ù,[>ßciff^Ù>æPÚݗÎ?gÇõþAŠt?b(yKftðAGN3FGL J0526.4+2247@fÛü;OagÀ¹¹"á£ôÀ9q—Å"/À:Ç)óë?Ýa`r=Ï@'üÆ>@<wà6a¿ë>ñöZ˜[¿ãô‰»fY7¿ééY³$°¿ÈŒÌ¡Ù¯UNASNone?ìÕ\™;®`?´E¾uýû?¢*Û
D'?£|'¬=?°?­¶çE:?¯®öòìðN?ì:#]/ä}?Ã;"˺º?'^ŒP¦xµ?›·´\Ÿ…?¹—BW=í?Á
 }z?çWÛC]!ï?µ"ñ@õh¢?¸V•î"GË?¦Bq¼Sâ?ÆuGüT5?°zÒP'µA?ê@°¢RX?·£è}Ýoj?yHœ4×2¹?`'£Ah?Æ3´YÛµë?·g)Çß.?î»!Q†6?¢¨ {Îí?ƒÚׇ$ôÄ?†GÚ´RO?ž®jÔ<Ë?Ÿ¢"·¥ÂI?îà5	w" ?«äØêê,?{¨8DG^5?‡Ï>Åw=Û?PÄ­]`?§-hï²ÉÏ?ì~(rmŽV?¦³¾{(ÔÛ?£8ԍÚua?•ãø†²¨?²rR#?¡ûQn­hÌ?íéUݾGà?› op­?pÚҟû­"?kLƒM">?¯OGϘO?IñÓÉAGN3FGL J0527.3+6647@b2(õ\@1Ä&5ïÀ:¼ÆŒ@ëƒÀ<Ü<¬X¹?Õð%cß@àà+yU?ý T "žX¿ïy<G׎?è«ûújr¿Ç4A¢D…¿×СõØ<UNASNone?ïøè—»q?AòéhÙûï?1Òü>çà¼?.}[é;°?Ct$Úíÿr?;ˆè o‹?ï3Úå<Š?›ÐFµä+x?¼À"®Æ?Bݘ÷†(?¦˜…cS?—›°¨²nÛ?ï¨]½Ü€?""8`×vÃ?…Çé{=¿Ò?uø¾Xšêµ?"†ÿ"<–?~}ù_äð?ïG'Á€_Ù?ŽÆ°ý.+œ?‡d7šÈ"?"2O!j!Ì?†·W÷a²?")éT5@
?ïûìØäeÎ?3S;Å,â?$rÐôœ9G?"Y›•?6_ÏD£òÌ?,'`eíh?ïÂÖªØA†?) 	çá?fÅQª€ëM?b"¯ƒä?s2¡Â`?yu6,F¸×?ï{D\6ž?xÎåãj=?{ȁ'ΡF?pü3´æ»±?ƒWnJd=ô?p
Ro5?ïÈrë¸}é?mµ¼zC7?sDÐ4ý`?cGŸRøiÃ?at!>Å?_LG›‰AGN3FGL J0529.2+3822@eFÕ䣃'@v @hÀ8éæè¹À;+%Â1?ï&gâ.@aÔ=ÚV"@D¡àe¿àH0…PXտ馃('ÄÛ¿êâ3ß´
¿âxC*¥UNASNone?îØ¢'€dƒ?¡6ÃgJb?•^$õ0X?—iîC/£³?QŒâŒ?'0xênñ?Ú:¯t³le?×
¢-Åh³?³ö¥=óÊ?³	6fl¼.?àcӞd?ÕEÛ&+ã´?éäÿÁõ6?©û°ó¤é3?±²a죵?›¿=ÙY—?¿% (I?£¡S0Ûh?ä²<Ì =^?µbє.a?¹ ¬Ížœ?±F‡Á}Ú?ÐSü1
Ü?²ó<]s{?ï%©¡"R?‹ÉÈ×úf?€OFºL!?'pA‰÷µæ?xΞH~î£?y a¶0¯œ?äþÎÍ-ê?Õò¼M×+ÿ?«Á¨,^¡¯?«ÿО'BÆ?Ҋ-`5t×?ӔUŒúNæ?폥˜'—ÿ?%òFÈ«?¡ãã«Ø?Ô¯«eM?¥ì'ƒ¢A?"PëÄ£w?ëfá":??¡DKç菪?­cãø?–"…˜ÿÂ?¶vŠ¾
?š‹U`¼MIXED3FGL J0533.2+5944@cõÐúY@,8ðAFmÀ9·´Ï€tÀ;"A® 9?ôw¬NÒöÝ@´¨€èß@¾?–Bø¿Ô:"´`"¿è
‡"¹ ¿ïÿ"[}em¿äüèjÚaUNASNone?íËÏMtkÑ?±ä
-­;?¨YÊ^u'?«fWã@׌?•Óü·Ž0·?ž@tO¸C?ë~bPN™c?ÇD€Tç?°°7ú±ü+?·ÿ8µ4?³\µ'Ù8Á?½LŸ''s—?é{{BãÌ»?®,^ż?¾ø/H]M?¦ÚŸ™h?µ+öœâ à?¡ÿ§+Õ?àÒAë ¹£?Ã÷ž%?Õ0CB1º?ǔ"_.q?ÂVrÒô"?´³%Ûiš9?ï[Ûíô\*?œ_St1°E?…ûýÈà]?—1ebñ—?wOî"?ƒê–S—k?îS'º"à?·J7j¿*g?™¶Q}y'?¦<AvXQ?œ†Ran&q?¬n÷ߔ†?ìr¹+B?£†ùۃ?±…<ñ´?y–ÄÓH?¥ÉîöÁ?"¨	ː·?éΉD%¸?±¶I
8Ä?Ãk>`ýŠŸ?°%³!bÍÁ?¥jr@"{?—v
¹¬'žAGN3FGL J0533.8-3754@nYcˆe"¯À>âôðØDÐÀ9ñjÉ¢uáÀ;ÇB??°ð¿ø«md¼@4¤m23@¾÷€—:¿Û·çÉ¿é$ {ÿ¿çô•qIw¿Ão¨{×\UNASNone?ïÛTDÙV|?p–T¼>)?Rý¡›Pƒ?T:Ÿ 1ÇÐ?k,êÞtƒÏ?lww‡(Yb?ï"Oú`¦?‡Uqtêé?fò¯;¹å?tP;| ?…}@&ô|?}
nøu?îMÎ@ü?"î£ô\;?'–Ç(ßLu?€ãñù1N?¡×ºšþÆ?æ3tMd?ï¨Û÷;x?€Úε¹?
åt©IË!?cƒÎ–s?…®¼9?€Ô
k¯I±?ïôZÂ:Ì?TÜx9k<T?8‰??—*æ?:ê·±TI?Q(,H =Ø?PÔJE¤Ÿ?ïÛÚ8èv?kíüg?Roã2ÙâÛ?P©i—Õ%?k¯3ñ1x£?e<Àhyà?ïZ¨qg!?#¤{ÉÒ?€šÑ"­	$?oëÿÕÔ+"?ˆ»%|'?|°ñYÚÌ?ïó5-x"?Q;wƒþÕn>ßUñ*üƒ>ÝÚƛݞ?YvO¥Ý?Q2À¯¯œAGN3FGL J0535.3-6559@q=Øâe,À@("_õIÀ9ÖÇÉWÍFÀ; dË[³…?¿ti"Ä@Œ!Ûé@˜¾_쥿åèå}C£¿âíɽJÏ¿é¯DI8¶³¿×?°=†/UNASNone?ï_7xðµ=?'öBl*-?b¤,Û+e"?cpù,FC?'Ä‹Io–®?'oV؇s°?ï,3¢nÕK?Ÿ—n''?v݆/Ü?"u[ñsBh?"Ù"Qco?šÕ6éü'?íö;»ÂäA?—y®xÁ
`?˜ç}ìÙ¡`?…îa'¯)*?¤(…MdëE?K l^²?íhº¼ÌF?¡Ä@¢Œ¦O?ñjTtXè?'2§…µ?²¼Þ¤,ô? ÷øP‡w›?ÝîU?´AÅ
¸J?_J¹´""
?"þ¥OëC?"èÁT['q?±Íô‹'?ï¼²ž€ç¥?'°Ô¼Œæ?`Î^àô–§?f`©E`?y?B³Jo?}"¯‹"§X?ïH"[ç?|  à?"wÝ\<?nIgƒñ€?‰‡¢36²E?tåà'ë?ïn#¶µÖ‰?~¦l"¬4?f[ÌÛ¥7?Y¿'7Ûj?Žà]º"?|[,4ˆ9AGN3FGL J0535.7-0617c@j=pdìé£À3¯—Ý÷wÀ9Kd'`˜À:ég¬·ƒ?¯+«ãõ½š@
¾‹Õ‹¸0@+Þßsîd¿ãb¡Õt³~¿çi¨$*¿ëE|Ђ¿ÓÕ¾î'Å?UNASNone1?Ü
I\?̦m›¤æ?®Øˆ³;'í?®	wÉ¡Zi?à
nÐ9¶'?Í/þôöT?îHFÍÉè?¶µöPy¡?p˜0]?¤ž¨ìÛ¦~?£CG|ä¹?°ŠÂ²Ö?ãéw_Tp½?¶bFmJüÁ?¸(؜éÏ?¡>"§)7!?Ò"ÛÝÝ?µœ8+P?ã·Eh-Օ?¿'íËþyK?"I…ªÛR¥?•r"Gë?×\ÜÕ-™k?¿q¥§Íl?è±²PZò?È	‹¼X­¹?'JÊ=KF?"ÖŠ´Ñà?͗ßîp>4?ÇKÞê3?ïuw•/I?›ÊÕg*O˜?tüãvGˆ?ƒ?b;Âw?ˆ?Õ2¸?•زPx'?ëxî:?©˜³}‹ë?¨<â~LҐ?"ëîå¡;?»…Í×0Jm?¥½Vµ0ˆ?ê¨ê$KŽÊ?¬§?ºú6?€e†~üä?s¦¦ "׿?ÄUÿw*?*?¬o¾
'pMIXED3FGL J0536.4-3347@mÉ{Ç÷zöÀ=o¼¡ŸÀ8¥»^æ?eÀ;‰al+¢E?ïÔ$
6°|@5"×ëŽÚ@WQ­Dq¿åøó	*(Ñ¿åù?®/—Œ¿âîü"þ"Þ¿Ò¦°UëUNASNone@?ïü´+@Jž?/HR_"ߞ?
. ?(ÁàŒý?3—¥,j=Þ?*·1Œbš9?ïŒ
Ðíï?ˆ¡ÿiŽ+U?i+nt¦â?t<݊Ap?†²€is–c?ƒ'
ÖЋ?ï*®ý¯?…nÐ_Ú[?…•ÿ`fÕÊ?r–"›}Jâ?"/½ÅuE?$~/Gûž?ï²q4ܽ?ƒÕB_!?<XAfÒôæ?E`'Ž7–L?'œaœ;ƒ9?ƒ|òpñØ?ïþB-é?© Œ?YZh‡´?r<)NÞÊ?!]àpä?õ;šÄK?ï×nç>h?n¢ú+*×>?T"ÃÂ9H?Q‰ÿvƒò?nG7ê`r?hÕ؉û^3?ïŠ12c:É?t¨á#[¥É?y7ð!6?e¹üi^D¯?€ì—o3!?n9dC¯(ã?ïòÄÚR®?_èØ¢=4?0¨¨ºÔ&?0® Ü'Nå?VM¤£ä/?^K0HœÎAGN3FGL J0537.0-7113@qŸIšé$òÀ?ŠµÃ›Ë£À:'q^-À;'lSq?ׄð4m@/ÒxÞ8@Ü )€­¿×
ú7œ¬ý¿ë³»õÔ¿êΚr1 ·?¶:,µÎU#UNASNone?ïžyNlí?ŽÂ«"èi4?hDe³­Û?rölU®%I?'nH55…`?‰€›	÷Ÿ?ïdk½›ßù?–€š­€?polÅá+@?°œ0¥u?Ž­Z4·"B?'"™].?ìêMœý—?žã
Mõ?¢"%‰£îŒ?''áé‹ìª?®Ç©ý?—:Wr`MP?íÕE ÀH?¦Ï{Ïjr ?oÛËۜ±š?~‰YR?°Vô¹'íµ?¦G:+Öæ?ï×՝'æ?"(²DÃûÙ?QÅ^ú"?zpάCh?o¢$ ôR?Œ‡W
̞?ïÊڃ³m?€u88›ÿ?\["{L§x?i÷Ù{h?så-…6º?v$…d¥f?îÀ*ðøä?ŽÄ`ÀÕµ¹?'mx4ŒR?'ËbÀ?–)®+^?†ƒO²6?ïŸ5ÐF~ê?€ôF_G$¸?S€Æ×´?Zl7bw+v?…Âs=ËxË?øå'58CAGN3FGL J0537.4+3604c@e ¼¾aÏÿ@h›_lw"À9ƒÓQKL/À:à«ÁºJ?à ¹ü*@
ÈQÉ÷/w@+ œ'­¿å ¹8ùÏB¿ã³Ó'7X¿êŽJÂ,¿Ý—…Ó>+	UNASNone ?ãK¬V4¿û?ÍEºÿð»"?¿¢¼©¥;Ÿ?¾Ý¨kˆS?Ñø)-1"?ËBËÄ0"h?àwª^Á_?ÔcñgÇöŠ?¹TWã?»ÊM^¶!m?Ø»•']½Ë?Ña¾Ñ·m??㚮O<?¶ ç\>F?À¯Âû½¦?«Nÿƒ¸™«?ЉËã©!?³Z›Wû?ÕÎJ×¥Ô÷?Ál
ó¬"?½9i-§>?¸7¥¥ß]?áq¶æ}ð=?':Öa?蔫fSNº?É~ÁH›?§W?Ö$|q?­´†ß¯?Çׂp»²|?Ƙ7¥dº?é/%é.é^?Í*S™7҈?ªÕa±Jæ-?²ósÒ "ÿ?ĎíÞÀ??ÆC"2?ê¢26€g?ªFùÁP™?¯TìÈ>?œf@W³ñ?»hÃҖÿû?¥ŠºíÚ?áÕÏÅ ¿?»)ü}¿ss?µÒð4œD?¥O!È	?ÖßÜz{?ºÎ«ZrxMIXED3FGL J0538.8-0341@iû}¿H€À1Ò=p£×
À9™AÞËÓÀ;2qúï?ò2JˆÎ@ž'‰±Å
@ƒßà›¿Ùb\ik<¿ìWG†ôž¿çq6Аj‹¿ïÿp'|¾UNASNone?ârþ•¥KÝ?ȗ̧…a÷?ÉÆBíÃðä?Ãó÷€/Õ?Ìm»¦ß¨?ÃÂzAU?Ã]UeãÎ?ÁœìN62±?ãÆ(I[yß?ÆU"ÇwÎC?͊	t¯´?ÁüTÏ»?àf¯Yteƒ?²þäá#m"?Ñ·@l	q!?° lI¦Ón?ÊöÁ‡µ?­3çèJñZ?ÀŠŒsÉÙÜ?¨"´€æø?á+›ýLŒ?¾{òÕ+¿?ÕcÊoû;?¹z=À4Jü?㨿±äÈ?ɲƢwtè?˾"=–?ÆB×)¥ž?Å ø'!È?½°CÐíC?ÔèƊ_â5?Ȭö2ÅG?ߙÄm"èf?Æ´óáï?Æúê>,G?»8¬?Ÿ¹U?æ¶~9ÊY´?®j4Cô‡?ǟÐÞ\õ­?§øÖ(Ѩ?»ltóG
? Á
.šOÖ?ωØђÚ8?«þ"O¼s?áˆJ:ÐzE?³iQT?ÊTþC+<³?¨± $óµMIXED3FGL J0538.9+1646@g³&¿‡iìÀ£¾"åÞÀ:ütðmÀ;t!퐑³?è«ñàØrr@ƒU@m-?þ@^_0çÿ?—µo	¹lg?Ü'§ÂYßοØeo™H™¿âÄz\¬B-UNASNone?ﺬÃå??'
¶d¿	?Xú›÷s½³?^‡uú©?|j÷ôl)?~õÖ‰ð?æ».&%{?ϗ÷Øê?°Ê +£Ú¬?®¨IÉm^ã?Ì®ƒ1^'þ?Êà~Àº?îˆk÷þ\o?'ø[³êY¤?'ŒØ0§>}?'™ôàøŠä?e¨Ô´?‹Ù4QOÚ²?ê/nb^D?®Ôàád…ý?·öSܟH?£öN-8'?¶Ž~˜UY ?¨ËÔ¾Ù{?ïä6oõþ—?o,|íV?DÆ~Aâî?CG"œÙ?f—ð'•ñœ?k¬êò6D´?ìh¢ý¤?Á«Bìí1?m²…Ú½)?žéÝ
hœ—?µcöFœ0H?»²Ö}5ñæ?ïf×áß?|Ñ¿âðÜ?€ºÞKÆñ?qÆwϖ"û?…)LVO*?rž's%ä±?툊Ž—f?"XYÞBÀð?¨ºµ¶Uv?‡R™'X·?‡Ã<Üþi?Šp)ÐâDÔAGN3FGL J0539.9-7553@qô¢}ŠÀ>–~
ÇÚÀ9ÐľáQ¿À;Â6âëC?²J…^t
±@SIÑ«@š'@‹¶W¿ç¼ŠM²v›¿àÕ6Ó@O¿êÉâ?Xc¿Þ~ØdÒßÙUNASNone?ïUˆÇ~+?"˜½Ž†å?'ë)Ž)³?†AQ܅k?‡²¤—v*?Ž0e­½?î´YV'ä?¬Ôâë©#?…zÊ"W֜?"@³?G®?ž·púj/?¥ÅWàØ­?íŽì;X?œ7­˜("?ž½»c£%z?ŠÊ13vˆ?§²`pö:Ä?"Ô6ùf]Ø?ìî›}ÁÄ?£Ø-Jˆ[Ñ?"(3öˆ¥?'­p7¶Ö?³‰q̳?¡å£oq­
?ïÑݾj<?~-¼‡Y?\rÎí¤ä?b%€ôU˜?oèÚ
ò ?y"*uí"?ï ö=řŽ?Wö}‡?j?ØÒ¦jâ?s»U¤åt?2zW0QÐ?‡ˆ':Å]?ï"£˜öÜk?''˜½ý?ˆóX¦0?t§{öŸ?Ždt?yÂ*›þL?ï[¶
Ø:?/
áIny?rµ¾¥"?b5±§RJî?Ò¢a¯Á{?~k,Iæ";AGN3FGL J0540.0+1208@h7‡?úÁÓÀ#¬U!š"{À:
ï°ýcnÀ;iþûôÅ¿÷÷äXÍ@œQþ'@ÛQŸÚÑG¿µf#@9¿ì{
jð—¿ÕF"¶U'¿Ó 'ü¨mÙUNASNone?ïÛ£ùZÊ? 7f(ëëþ?-C‰ÑŒJ?,T#Zb
?qDU"Žò<? 6ƒžÖPv?«?©è%•Xi?{:2ö¶L?…Â
e? Ðî–Q<?¦£óA"y?îyGzצ?"pù	³&?‰nYœJñ?xa²¸Ô'J?¢+ô'Ú?'
zhh?ïU…w<'E?‡Y}¯43Ú?ª(m×U#?	#S›3?•F|@(%?‡T…·f=Š?ïÑv]¹L?¯À>H5?FÏ~É@Ç?‡jˆ¾ì??tjÈÝ_?¬7fÁ?ïŽ:	*?"àÁU³+_?e1uñ"II?l92ºá¦?‡% *TØÃ?';ÿÄø–J?ïiÒw£?|ðJÓ|?z:dìp›?h†ÃFÇÕ¹?ˆÜ¦1ù?xx'ëPÊ4?ïܒñƒ>?_@ËË
»›>ðŜtüœG>è¢ýà.î?q¥ÁܵùN?_3ÛØæAGN3FGL J0540.8+3503c@eÈ}¿H€@Þì9yžRÀ9QؗÜ*8À:Ց¡}"ª?×týý`,T@
ßÈß'·@* À){N¿¨Q¾N.â¿ë‹Sß¹¿èҘ–dZó¿á+k4›,UNASNone0?åÒ{=õP?˂¹êX40? v"£++?¢»t¦>Di?ÒLFQjx;?ÊÈm,(R?Ü´¼`Õ)?Õ¦Tž<ì?²†&Œ¸ü?²ÞKªl]s?Þ©º¢ÑY?Óý–̾<Å?âöyw¡]o?·‹»)?§?º™eŽœ‡Ø?¦JP­­ÒÖ?Ól³­#-?¶É¯.À؄?ß¡êWïw"?ºÃá86Â?¤áÚb"<?Ÿ¥ž¦/?ÝÁÚ[çÄ?ºþf3 û?é2¥æüEX?Èaæ[átœ?ˆ×'¿m°á?ŸéûíÝÐ?ɧõèO	S?Çÿ!{ÙGã?æŸÄ'&ï¿?ÓHŠ8ä´0?§:`а?©0êbÈ?ϼmjLá?Ñ$—°F•w?껹¤xƒ?©ªŸä?ªë#I6»?—§;¾~¿?¼¬¡7Œx
?¥ëx'9¸X?ç…=àœs¥?®rt!÷î?ž­oí×<?Šl+Â郙?ÎZ~Ài+?­YƒÔïMIXED3FGL J0544.7+2239@g(-¡"ú×À"ôß:›À9m"š\7À:Ȫ-e"Ù?Ë%Ì~"{‹@ûäêû¶ð@ýÖàL'¿ëd¯N"¿ìiPjjq¿ÐŒ÷£ÿ½Õ¿æÝÎzªsºUNASNone?ã‰[Åï?ÎB˜"Ãq?v˜N|x=?z"`Ų±?وŒ1:$?Î@t†²¾?àðòôÌ?Ó¿¾Ø~—ò?²óÕ­È°?±­ˆÖ"&?Ùcó—»?Ñç,gš¡Š?âía ©‡?·z‡qQf?¸Té¸)?£êgÅêŽ?ÔN¥:É?µ?½·qv?á5sƒŸ 0?Åpû'd@>?Ž2—ãÔ(Ë?*ZTߞ?Ü£"95*Ú?Åm͆Â8?æþ…¡7?΋y­?l=¶²¾?sxw>\¨i?ÓÉ©ÙÐ
?Íúß  /F?éGwÂk?Ïå›ãÿL?¤!¢ˆÌC?©–³ ?ÆÊ{‰†?˲o1ÚJ?êP!wìB?®
qs	âØ?§W%Ò]Á?—3·2Háø?Á¬ö›¿R?ªFL\ÓTK?ç3A¾«?¹"@S…¢½?˜zƒSÜöæ?†åt=³wŽ?Ð!GDÚr?¸Å/[£™íAGN3FGL J0546.4+0031c@iœuy(àÊÀ,Q3ß*À9g<kÁ:À;!1ZL?ëj¾ÿs'@Îìt‡ç@@ŒTçÑá¿ÞxoÖ:ñ¿ç–¢ˆƒ¿ìxªô_ãÀ¿Ý)1þûLUNASNone ?ït/Zi?œ±n㽞?'¥zÐøù?—\ƒ·Ñ?…Eã®?‰{‹Ô™|?íÆΫºI?½j~9
?""ÌÆ»½e?£Uî>σ?©H®è²ÇÃ?¶ûÍ~¬?ì#¼*Æ°²?¢yUe?ª°ú5&?•Ö毋™2?±‰¡…™o?™¨†¹›K?å$剿º?¸¬1SûxÞ?±|s˜#?¯Ï
=ö?ÑW¿¦Ê?¶ºMwLÕ«?ï¬Uýý59?ëˆ)§¿²?w'[ãM¾4?x…"¾?rC¥
ÙÕK?qûS¡©d¾?ï='
ÿ?¥HLP©?}E;8²Cu?‰ ¨öf ´?üÀõ? 5ßâw?îzpe‡ˆ?'äù£ÌK¾?–Ù#kk¾'?†m1J?™ØÏå[?ˆóö­'Y?ëÓ¼]L?£Ïrké?¢>ÏÐ` Â?"—Èv5mH?¸B¸®=?Ÿç†4HAGN3FGL J0550.3-4521@o}n—OßÀ=H¤TÞÀ:´ƒ)ìÀ;¤B"ÏÞÀd&Æs@üЉż@C )"¿çbò†ßû¿æÆ'Ûjþ¿ê¸NÉøÃ1¿à"}ÊþcUNASNone?ïù½æLr?Aüž´ñ÷?9ó˜"¢?É?8뽐Q'?85°ÆП?5‰:O[¸?|+…Ñ?‡âÛý£K¢?gxçôû¨?uOhNš+3?"Y'±ÚZå?Å8Ú=¿?îŠæ`Ð-?psÛnü?ÔQdï?{4´p•(n?ÎâYY–'?…±ûÍl?ïÏù›÷Ô?FýiqŽ†>ߒ
€lÍ>û®£+®?wûšP/æ ?DÐ.(?ïü˜¤Ép?5ìãJÝv?)r›s¦zZ?%ä%ñÔü?2yíl؂ý?,Š||ÇÝ?ïܗ'èþ?mAàªb/C?Rª?Q,Ô,hš?j\ô?]*?gž% >s?ïci3Ð?uý³M`4?€úN³<èõ?kµ³Ê€ö?†+dz‹¼?j¨ÒcèòB?ï÷êÜ|²?P7G^ü>‹1¼(­ÞÂ>¶ïSwÐ
?P+.³?P6Û-§+…AGN3FGL J0556.2+3933@e~P]¥@7.jwÀ9-—ïunAÀ;_	ðCÊZ?Hږ!\¡@¶†ü#»@¾| aõ>¿æè'Wގ@¿íbääúƿꄉðŒÎ
¿è=¡íêÃrUNASNone?ï–ÐzðûÅ?†ug''ŽZ?uÝو4?s±hïdï?~º¤¡u‰,?»ò+ €+?ëZÊìe¤?Äî5)yîP?¡Ö¿WØÔÏ?©N`[˜?¼>HòÚtø?ÀV½ô?ì)Ð+ƒ*?¤ÝOäµDó?¢;Ɯà`?Žw[éü,?µ¢á"ç'þ?¡‰—eV?蔆ωâå?³OO¼‰fN?«ÃA˶Ô?Ÿ0´§ך?ƽP¢g?²»0Iô?ïÝOøw×?qÊ/ÞôÓ`?XÊå^™‰n?UY÷¤†Ž?fJ"òj"?nw7ú²¬?îŠJfÿò?²Ÿ	ï7É?‰éyjtôç?•éü&]l? áA†x¤?¬r–¬qü?îeµÿg?•Ho?'@Êå/ÞÚ?…ΘÈÇE? Ï/)m ?'?£K«?î¼?"šØ!Ù]n?‹ÜÁð!|?vB»–åy]?§Ý8|ô?'øáÈ+AGN3FGL J0557.7-0720@j®›¥ãSøÀ.}Ñ¢£YÀ:->9 ²þÀ;oX)ŒÁD¿ðä/,=u¬@ü‡ÝÚf=@/;ßÕA¿éâ¼"ä;¿Ó õjÈS¿çà´¡ÃðÁ¿ÆçãUNASNone?ïܸ·¹a­?j]Ӎ¸½/?X÷¹L{?X5ÅYDû—?fˁŒGL¡?e•L©	!ß?ïEèðÔ?¦*z¸?uº®}Þ}{?"@«Ð€›ÿ?'ïWI¨?—Ž¨Ó2?íº€»7ŠA?•4½š"ð?š˜ÉO{?‡JØû¶Ÿ?§¾m?m›¶jºÓ?îŒÞyÜe?š7˜³ð¦Ô?Pv†ôÃ7U?Vr?Åt2?¦®d8Üü?šj]8a¾?ïï.rÈä$?\¥™oŽÁ?Db1*-ƒ^?F€[þôõ?Wrˆ–ì?U±i3f?ïÆË$šØÎ?|ÿã¾%?\´®­Xçm?c6:}kû?umB"<?w†~]Õ?ïx**˜?ƒp]xê—?‹0óºbÂ?zúûo?w& Qä?vŽQđ?ï©Ÿùã?s´S¢ß?*ç¾4XèŒ?$\?…QyõF?rù¤$ñ©¶AGN3FGL J0559.8+3042@f!ê5"`@~½à ¿(À:+0/r´À;pê‹út¦?æjÞu–°@
N½u@ô½?û`zßDH¯¿ïÿö(výÊ?ïþ`  =Ú?cÝåÉQÿ¿Þù…ét´nUNASNone?ï°ò¿XM¨?'Ø5m@?Vow¢ôð+?UÁC¼R?€õa0˜!?Uõ"2&å?ꅭ÷I£?Å
ÛN´ˆ?¥RíO¯x?¨[J'Éã'?À"ŒÎsÚ²?Áх#ñ?íy±ë'´X?œÍÒ`~}±?"Yû;[\?ƒÃ0LìZ?®8XSV¨Ô?™8[?ì<'oýá?²<ß\é?ªµy"o…c?§ÏK¼ÓÜ?­6ÄdØΌ?«
bA´B?ïÚ"QÓK0?tx{Ôo(?Dñ€zi?Fk]QÉH'?pP´L—?sۓüW?î2od¢þ?±±s{†?‹bÐÎ:?Œ÷ß)ƒ¢…?¦†~-N?­]4'ºâ?îÞº;–?7zÕ.&K?"à1B=_?uÕ	y ?™ÍPb'?Œõh&£æv?îJØ»îX8?—Ñ5‰œñ?¢!{€Íòq?Æ8¾Jn‡?'añ"°?‰½ù<šÏŸAGN3FGL J0600.4-1934@l-1;â.^À3¼˜å>³šÀ9âÆo»y¾À;­1"́þ?ãٍ«d@®Ðǃ@r @§ºï¿è~u΅«ó¿é5Íí3J¿è&s†¬ÏN¿ïÿHÔ|¥UNASNone?×ìJ?¢€/A4s?ƒ§€8ÔÅ°?‡–Æ«u?¢jÒs	Iñ?žØÓýI ?ä;NJÄR?ÆÅHðšîj?É
!.'©?½Lé×cm|?Æ´³À%8?À5œét9?ëâ$.3?¥t'ݦ ?±¯¬L'?˜ï;€—f¥?²QB"òbU?šIè™k}P?âã!'öq¿?±mByn4?Î	Nâ€1?°NÆÓâ¶[?Æj,}¦7Ñ?ªˆJ)Ùh?ïq­æÇc›?Œöés$#œ?s§IÉþ=?u)œ@Èß?‰ÀáÖ ?†åÎàÕ¼?ëkXƕ¦?¸Tƒwq»)?²×,"êÌA?¨°
5ˆþ
?±Î
Eúo?°é k?î¼ó!0?'#!ý‡¨÷?¡H+J®x?†]»¢'÷?™Ø
ýæÉn?'eKÈ!4¸?êПS±œ´?žÑìd\£?»[È_¢p?˜ŸF~TôÃ?¬>z2[Þ?'Û-Ħ'
AGN3FGL J0601.5+2309@gYW)²€ñ?ÂÀË6ʗhÀ9N˜0
À:íÒä>š?ÛËÆe!@—ñ5·ÇØ@àšüI½¿å²y3‰æ¿åKt­¸¿éc™Z¸¿ç€ †eéUNASNone?á+Hpå£ç?ÊPVÇ.tª?¡‹9ýÕ?¡ë['Íҙ?Ûxý¿!Ø?Ê¥ipÃ?¯ÈK7òò?¹Vï0ª
ä?ºÿ"[/ã?²H‹]ar?꣏EÓ?Ám 7[?å¤f&ß=?¶{sí!Q?·›zHµ?V?£p¤Ÿ/{[?Í ª£	ãa?²§Ýá|o-?೏œj¯K?µêcù÷Ì?¶–­…M¡?¤z•€¨G?Øó5e×9&?´xPGÇé?é¦yT»Õ??ßþ( ™N?ˆ˜¯õâ«í?‰*ÊcMô?Ç܏­²€E?ÈÅT+$?ÅHgý:6?νNIäûm?»?k²¢÷^?§žÒ–úÓ§?çEøŠj҇?ι™`±)?ì1$ûŽL?¤°Å/I™§?¤•X¸ý?'MeH
.?´,,‡? '^ß*ê²?çïž+œ?§Õm/X]?¬²:<vYÍ?†[Z`÷ü?ÉNùëÇl?¤Crƒp±pMIXED3FGL J0603.3+2042@g£ùHUÚ'¿æðí=…À:c–j:0}À;.LC¥q?¨âg-¢Ê@	ºRøöKv?÷ÿŠŸUÆ0¿ï|	›ÄC?ïqlÜÍ ¿µ/µz¸½R¿æb"¬
ÔCUNASNone?íœ08h7ˆ?»ê°ç­½'?hˆïò$?qS)H$é?²Z6´Åð?»¤pLÌ?ÄÑ›¯ôO?Íýëyql:?Åáeáhö?À¢	™u¡?åSd`Ò¨¯?μ ô=C?êè6ífö?«m?\W?£Æ&ePƒÿ?""몔…â?¾Û;ÿ¤TL?¨å¥L/wu?ç0œýç!?ÄzqOyê?¸'ò"Ç«?´Óâl{'6?Æõ†öÿ¦?Ã(qÐÊ)Ò?õÝg?¹¢âê+¾†?]ݕ3Ò½?eé`©Õ{C?­¨šÆæv?¹u³ë¿?Õ&óuiI×?Ôø^ó¢Æá?t?¸ID^ØI?àÈÃgÀ¥ï?Ò(ƒØÎI
?í#Lò];?£²ê¼`"Ë?œ¡åjól?"	…Ú?¯ÌØ~dg'?ŸáQKô‹ˆ?ê¯67PÇ?´?qF—?°úǬ	Ñ?£RÕR$?¹‹ˆ%Q=ø?±<
ø9MIXED3FGL J0605.0-0000@ió(àÉÙÓÀ$š¾'›þÀ9"àê'À;Xƒ°j?Í*™où@—8v,®@'T"¿Ò@C"OÇ¿âR€"ÁÆè¿Þ{>í¼¿ØèÛ8þ׿UNASNone?ï¿é½¦ò¦?t|~ŠjÐ?_<Ǻsî·?X*E>%
?x;ï9Ê)A?q і"O?íŽÀû2eÙ?´ûÅÀ‹mS?‰¤°ÆSXd?Œi>Tpçì?°UbÈ'ª?²º"Â9Nj?îœA/'é\?g•\ë`?'GM¨q§!?ßGÌe?›0Œk±õs?†±Ôira&?íraæò4]?šÎÕ­½?oû('Ë?m AiÜÜr?³m§k¿A?™v¿YGj?ïè݊ÆSG?Y&q©ô"D?Iã:¾¦­´?A´Ëá"?`©¦ÈÒOl?T»òe‰Ü?ï ý¥v‹f?¡ªÁ#ë$x?uo;®S?x€Û2ÇL¸?–"|'Qð›?žº±ƒµê?ïpœÄ,¦?zWW™Å€?€ç>Ù}¶ï?t5$_'Û?ƒ™ïŸÉ€?j¦ï|Qð›?ïMP8ã²~?y¿åNöø?e}Ddn´?S'M-yò ?"¦PfhÍp?xœj8À×DAGN3FGL J0605.9+2039c@g¯Þ¨—c¿Éß8IÈuûÀ8Àº;А§À:¤®á){?ô¶@K)t@cä¼Î@Þþ€N?ÎR	 pV¿äùóK'£×¿ë%Ʀˎè¿è6­Í>sUNASNone ?ÃÌTÕ¢çÕ?½ò_0Å£?áJ;`d€?̑æiMmé?Ӆ›mÃ?Éuåu)?‹³û®úÖ?–¥äØ;¨¾?Èæ)àN3ë?½ç9#{ôÝ?éW¥›…'?À+ôÙ?؝rß$?¶›"³á÷à?Ì¢\¡@¬î?±$ÀÎ*´£?Ù^ÐM"d?µòsª"§?ÃeKZºQ?¬ÀR2UQ?Ö©8hQM%?¿Ÿ}'If?ߤ!ê­Õ³?»¨ìYV:?ÝÊcő?ËEl,	Z?Ø)ÀU¡µ?ÊÞ­Œ?ķʺ¬l?À՗/˹k?¤;ƒª=,'?°®ÅáÝ;k?Ìí'©Dåì?¼Zì9Š
?ç€ýÛ&pœ?Ã?$ُd?åäÔ¼–…?²­"Ç3?Ã#Fe-ðî?§^ 2'­?ȁ&Gß´þ?¬Úæ?ÑÂËË´¸ž?¯_\ ?ÕÇP²±(é?²Ä¬úí?Øuずz?¯PÍøÆÑMIXED3FGL J0608.2-2306@l³­À˜$À3hOô4ãÀ:r(œ×;¼À;áàÈðŸ?àùµI^ª@
úp­½@štŒB¿ä´×Qyß¿ä@¦ñ›ä"¿ÌeÔ
È¿ïÿ£©	pŽUNASNone?î'}Œ%p?§ãžC¤#ô?"žÞN•¿c?ÕøÂ	z?¡È0'"%?¤Öù'õâû?çÆ×ëÂcñ?Æ
B-÷ßö?À­z÷íâÇ?¾¦"OìŽ?À7%[.Nó?¸í%qy?éÐoÓU?¬­ö4.˜µ?º5ÈàjI±?£I–楫?·IöÁs*?£AËð0?ë%öĚ?²žáº?®Ï蚂?«ÀåÄݘŒ?·Ä(Áó³t?§=ò³I²?ïlüùC
?™"hUŸ†Ó?kwsyÖM?p‹íï'6?âäÁT+x?˜ãtð|[?ìÇw´9ó?´ÁÆ.Y!?ªIø¸ì?¨þÚ>Ç?©	DýTí?¤cA
9Ô]?ìÒ9}q'6? f+Ø5³?­2Cïœv?–nwÈ\§?¥ª%Šõ'?•ú¼ø?î#XMë?–÷¾%?¢¥¨¿©*?'µL¶8¢
?–Ižg[DO?ƒ¼)ÈŐ÷AGN3FGL J0608.6+5328@d	 {5*"@/›Oe™À:Ʋ˜¬À;œnCªy¼¿ë½ñwÑó¨@áÖÚAÕ@ðºà'$Ö¿µG㈿àŽæ•ÔF¿é¤Î#"¿ã'èd6¿UNASNone?ÀT
?'¦@ J†?~ªjMlS?‰þò£péê?p'5ägÄò?'÷J‰ñó?î»åkÕ=?¯6Õ˜?ˆ…wF¡?'ÅÓI÷]?œ4I¿?¨ë^n† ?ì©ÜlÓ?¤ýXfî?©!Ò§q?˜r³{Âîý?²' 2(àä? ‡ÕánPˆ?ì½G¯Ó(?§§u±OFN?7®/7W?C²ÊQ¤6?¶Öõ˜éˆ?¥×±›,¼ƒ?ïêïǛ?j±E…±?Y(Jn²"ý?cHXñ8?Pø&PLwÁ?XŽ½Œ®Ê¼?﫛^ëÈ?Ôªh~+›?m^ ÿÔ]þ?v¹Íœ!?{'ÿïyøý?ˆófYLä?în€¤ˆ¾‰?"¸Íâ,¢¤?—àÀ#åñ?‰=]/e[??šO+QáuÜ?‹Àa3À"'?ïN>¶ì?'á†Wôcå?_OSÓN`?Tv=tKÍ?"?H–üï?'+§ß¡ËAGN3FGL J0609.2+2051c@gµzáG®?âÎìóàÀ9-J´O(À:˜}–-ÔO¿ãoXš9Á@
n¹?!@.'`@3¿Ò1#"Øå_¿äÝ÷½l4¿ë°²@jºo¿Úð¼UNASNone0?œO£Îž+?ÂlÈ­ó?¾Û®keî?ÁαDlR?ç}vT^ë¸?ˤ	ÎÏ +?¹|•ùò?Ä´zŽšÇ?°5ìB€O"?®ÉL@ž¡?êÉÁd¹½ü?Ç	i=äś?׋ùcêÇE?µþ–ëÅ?ÂòŽ6}Ú:?¬jxâÈjE?Þú¿€ÖKž?·tX½<~9?ß_¾oD?Ä`ûF̆ñ?ˆAWÐH?‰Ëq[v™?ßÞ6ؕi?ÄZêbÆ?Ó —n_óÊ?ÎnH_6¾¥?´TY]9M?º'ƒ…j?ãå)
_˜?Ðó%Ä­?Ì"ä ux?ÓZT€œç?²\ã]lsš?¥'¬Q˜~0?æ¯>ZóZo?Ҏù¨"Œ?ä ¬gãa?´É {Ë?¹DŪ4?¤?£bìHèý?Ðmvkþ<?²»—	£@,?åò›Ï–{?º¦ë‰ì?sw±zõ?g¦ü^'è¸?ÓÌìZK@?ºi¾í]ˆiMIXED3FGL J0609.6-2851@mnµÇ͉‹À5/.ÌțÀ:J¥öŸ..À;æ,_Ú[+À"¦ÃMÈ@	A–xQö@ý`O¿èT-ĉ\`¿æZýñAѿ㜒i=u¿ïꆳ&Í8UNASNone?ïå¡14ø¨?h(‰k?YüXa³&È?`´ðÊôS¦?ZÁE"™‹?\@ûð<BÅ?ï Tž4Uj?¤o2û›ex?|Q¾ò)å?Ž´¦IÝ?"á*ý©`? dziý?íh³º¤x'?›k‰âæÀ?¤úN0Ä×?…pÍ›"?¤z'?†J(©S?ï3Ž†QN?"%¾Bt?VûÁ2Œ¦?fòX»"Ù?˜s(XÉ!?"d^×ÚO ?ïïÜCåT?c˜o2÷ÓÓ?Pj$³~ø"?`'é!šñ?P£DÎ4ž?I5Ã	Þ¡?ïŸÂ}"?'4èøû÷?aW=yi?¸?v)ˇP·k?vé´¬ø?v<!§n;@?î´7ƒ`-?ˆ2+U¬|?˜5lj­B?€†dN"UŽ?'I±'wÉ?zJqKÈYŽ?ïÚH»°š½?mÿ³·ü}ä?†è8§ë(?-÷Ñ
i?ru†žxÿ+?mÌÆøÐ&AGN3FGL J0609.7-1841@l.ÄÑ¢À1bÑ9C­À9¢aÅíµ{À;›ÀoÇ88?ç	ů)×@~ÛËÃ7x@cËè ¿Ó;ùæ`q°¿å©O°´¿ç"Ky¯n¿æµêpLšUNASNone?ïˉNÙèû?vrü°?ý_?rØxèÌÃ?s°ßኙ?]4‰‡L?V&ܞ3)Ì?íÁëöïÇ4?·‰¯PA	?"T÷S3.?–ßò"ڐÿ?©™ɏ&?³}KøTy¥?î"+¥9#Ò?õ%l²A?–Fã³&7?‡Õú%?™3§{š?'ݲÉþ}ª?ëJeçr~?¦¶½Ï€q°?§æáÏR?•ªCÌ7Åw?¹äÎSéÞ?¤ƒÎ:¼èŸ?ïîɔç‹È?^éC†U°?UxGÇbRL?Y7¥¶mòÅ?Ié‡êÛ§?DãÀOºK?ï=}Ó¯-ï? hçBÄÌ?|ä"P뀛?~"ê%ô>?'$nP=ü?šÊ‹M'Zu?ï\Éé‡\o?ò»CÄm0?†CóIä$­?|¤­œwnÈ?'‰'X¼=‹?qSÚ:¦—?îš#¤
՚?‹¹ 4+?"Ì}$-h?v)xi?—ïdH‰D?†m͹ÔAGN3FGL J0611.5+1957@g×.œË}A?丝jßrÀ8Þ$ZR[íÀ:¾Dä5Ÿ?ôjÅ(=¶Å@³ÅPÉ@e@v'®¿ÂtÂvÔêö¿èvssârH¿æˆÅ(
,¡¿éœuʐUNASNone?¹9%)t?³—`?—?Ön‹)zˆî?Êc'ªòe?á•F?Ë\Œ¹Èt_?u&¢Ñ)?™»I¨Ñ¬?ȁ
¨5Ï×?»«¶DÓ¢2?é\%Pòa?¾Kbæz?Ú–‹zЉ?µÐ±"–:¼?Ê^îp?­ÐQs<?Ø3\Å"¿?µ†t­Ó˜?Ç:&ćPc?­o‰~-'?ÒY€æ€Ž?¹wt»Å?áêjë ?¶}=ÙA‰¿?ѾIô(?ÃX_p04?ÑʏR:W?ź8XJf?ÝÔw&¹8'?ÉF…ǘ?«·NVíP?³š*G®Ã?ÍÆßԉ?¸0€|E?æýٗ‹wm?…ʉ€?æ¯X̔?°à{¼.}?Â'=†ž?F?¥ÑØ¿
5a?Å^îŽi?¨°
;›¡,?ӕØæäs?¯ÞŽG)Tû?Õ[ví¶ëÿ?°a!w~O?×°,-/Ž?­´#	MIXED3FGL J0619.4+2242@g¥Ô¿	•«@l'"øÀ8åtË"¾À:dX R…ß¿´j摏¢@Â]](O@ƒ 0w¿æsñœ÷¿àr¼‡Ò".¿ßNr\q¿äI͖ÑOUNASNone?å]菺·e?Èê^‡c¥Ü?"—‰1?ˆg"ƒ
å<?ÔBv—¶ëd?ȶˆKØ4y?éîÛ²îªB?É+— 1?—®RÁÌq?›d±Eâ×3?Åc›iíi?ÆøӐá9@?Þ³HHæp.?ºãç«Ó?±'ÆŸüD?Ywc»?ÜèF0Í
¡?ºƒŒo˜?â«GôW͔?Ä\•éG?yõ!üfYÝ?qTWu¨¾?ÚA›×½°?Ä;ú?ëÆÙ>†^»?™Bló/?"(²uæe•?§DßæQ?¿D¿ôö?ÀõgQ.,?îi}—&ïû?°Ä³X?'"}Õ**×?ˆu xØoG?¤ß‡Š'?¬§
M«?åæïÐø?¸%"©rÂ?«2gi*?›NýAžUÍ?ÐÑAüw,?µê·"[??çuNØøw?¸zV%"&ž?€b©Õ"PB?k*¹Ïàv¥?Ñn CA?¸&Ÿ$Ö ¡AGN3FGL J0623.1-4143@o1"…]¢sÀ6ªk\šÀ:…vWu1ÛÀ;âº5"¿ã¥®éjšÜ@©'#Sl9@R?'Kõ¿í^¤blÔ?Ï(²aøª¿äc•åHÞ¿è˜Ò?05UNASNone?ïvÖI‰r?"–°ÌŠ3?‰‰É—äÚ?"òk/†Z?qH\Ӈ?kRwøÞCZ?íDsæ	ge?·11˞b?õ0n1áÏ?¢"avg]?¬¾)hP˜Á?±¶±›Å£ ?íb¬N
eT?™±
¢»ï>?¡-Ø^ ?2mxnö?¨§búA"?‰
3ʍ?ìœèĂ®ú?¬S_ý?«?›€R
?¦I-åNJ|?ªòaœðX? ^6ˆ{"É?ïÅ(Ý*#P?Žõÿú`S´?tzß7:+X?Ž`t	K­?aád%oÙ]?^"²NQ?ïQ•ä$ϐ?´è¸7TÛ?|‡X­»;?…Ùô$@j?VÚî}Àƒ?–d뭆¸ ?îò"H¥=ð?‰fØQ:ZD?9áÓ8.—?'§¿ïþz?'sµhEe?~®	7ÁP?ï[•5°f?'±¼>?{—…Òñ3É?s<"]?‹NÕÑf?}úf¾5ÔAGN3FGL J0626.8+1743@hLœàuöý@
eä`gIÀ9;\Í`qÀ:~·îï6"?ôKg<O;§@&X¹Õy@˜Ëßçܞ¿ÛWÈ¿în…(jϤ¿çm+?Úò'¿ÄÒ*Þê aUNASNone?ƌyþý)??Ç#Èý4s¥?£5}¥ka?¨?XäÖUx?é)ÈÛÚ?ʇ¶#Ç?à 
¿¹Çj?ØrýšíN?©yi&Îå›?°ö°)Ũ?ܐ·[)$?ÖóìÏ7K?Ó¡¨r`«Î?½3Ñ98Ö?ÁlË¿Jr?§¹œsRs?áÓøÖý
™?¿µ·î‹7?ßÚZ‡?Æ×Ð]óÑ?£%Rª.ت?¯Z»
Î'O?ޚ{'ƒ¶ê?Æ÷Ö¡-?ÎW>˜?Ìï|ø× C?¡Ú™øÕ8?£¹eØE'²?çaÉ'Y?ÎÚ½4m3Ï?ç]µÔHþ2?Õía(?? «†áCú?¦ žÂ3§Þ?Î^FôÓs|?ÓãM Osä?â‰Ò¶¾?ºªÓ,&=p?¸&2:ç?¡1ہ[åM?ÔâΙ«7?º20þ¶»?æÓÆwYd?¾DéS–*#?ª
KvtF?¨•þcۍ(?Щk"ï?½·ÕMIXED3FGL J0628.4+2429@g'^_0çÿ@ÔÃ\á'fÀ:û¥þ+êÀ;\nªƪ¿ÛLçDd@
ç݉Þe¦@¨‡Ÿqü¿Ýp_
ô¦¿Óø¬
ÿI¿æ=î"2	¿å‡†UNASNone?îÐðçov—?¡,H«'ÿ÷?}í-º€H€?€x»"4n?žf—¤üî?ž¤^Áæ??솽iFY?¿˜'©íz?'P)P?åG?—ÃGŒj?·w÷¿Éìä?»áÝâì_?ì]0>®ˆá?¢h{; À?¤ì,—ñJq?Òà±1ðü?² g¼ÛE¿?œƒ«Z\#	?쮗Eè}¿?¡ù&ãgŖ?‹^~;µ²?uN)¼d?·"¾ÎÙÙ?¡,ïTꛝ?ï¸õRäÄ?ƒŠü¢©?^œ‹"­
?a-˜õ(?{Þ3Éæç?€Ò
'D¨M?ïb/à?¥h
‹†ç?xÝÏn ?@b»Ÿõr?™…M8@Y?¢rž?1x?îÄ%U\d?‹ö	•,?'mœËGS?€}•ê$ÿ?–
¿­ÀÈ&?ƒâ8ß7?ïá]?'\"³_k0?oñX`HF?\5ˆ<—èl?›?Ò¸P[?n¬|¾v,AGN3FGL J0630.2-0929c@kaЦv ïÀ!öúaZëÀ9¤,ŽÔCºÀ;5,)Bï?ò>»Õ-Ä^@!\q@ñgya¿k²ú•gC¿ìÒ
}¡/T¿âu	u…ÏI¿ïÿ'?¼UNASNone ?Ú<
;‡"?ÇÌö¯/"(?ÌÅ>¬Ъ?ÄfnUëfb?×aVnn'?Ç;&ØÃi?Î&
F¼
H?É\>‰ƒi?×_|ƒD~Æ?ÄLåXVP?ٍ~Zp[T?Ɲfî ¯x?Þ~ÒõAd?´Xûáx°Š?Ӟßi1œÛ?²ŠA;MwÇ?ËěC?¯¨$ÿ,?Ôcü¢0´?µÂ…YÈR¨?ÔOŒ&¶Åq?½qˆ"ŸÅê?×Lw7Û?·ò›ýٛ?àÕ÷náà?Évà~|Õ?Í:Ÿë Ö?ÃÙÙ$Éãä?Ïq¿€3-?Â:ñòa?ÙÓЌŸá?Îû=x†y?Ôº"-v?Äi.å5Y?Ñr,ï2Ž"?Âõ9Íö¡?å·YÏei¢?±-ßxîJÃ?ËWÿ:³/B?¬ˆÃô¼?»•3nTi?¡Ã:éAŸ?ß-`pƒÛ?°Œe✒©?Ö)q[?±¥8ÎdžŽ?Ŕí
"?¥""é&aÎMIXED3FGL J0636.7+7115@añ~|áœ@8mDþ6Ò$À:
{À;ÑïSàQå¿øwƒ…*L@Ùº÷7Y‰@ڊ ,…Å¿êûRAsñG¿äNnU>¿ãš'"¼²p¿èèÎ̶IUNASNone?ïübµ"'?6›s~	Ž?(søB[Z?*¯'¼<q?0°X)["?+ÄD9¬#S?ï«B¤É?†Fc
VÚÌ?pÿeQn¬¹?x
+Шûh?y
ó!ç?€NxV{~P?ïO¾·?€³–/UÒË?~N ðýó?qN'Úœ¼ä?Œé.}[t?yfwâqp!?ï»Ë¤r†?vu"µ0¡Ò?9óU$sü?>ËX|eÉ?€=|)Gª??uìºènŸã?ïýËßUÕ8?)îö^*A?!ßçzÓ?¼ˆRw=U?"%(èÞN ?Dþ½_¤7?ïá']šÃ?h7ñºÁ'??YAaùŠ!?SÖº3?aÝHqf%J?bãNºj]?ï±ÅÉß?q>ß©"JÂ?o·—´+?gœÏâÑ?w›¥{7Î_?fôÂPoH«?ïôz—º‹?P­œÙ¯¿?
'‰ƒ•8?¥ÙxÄyä?V<	ÕC¤?PxrŒ\îAGN3FGL J0638.4+5704@cÍ|ßýa@4ϋ&9O­À:Á=L'©À;íó?']<?Ö䟫›=¢@}'ûr|Ÿ@jÎ]=s¿ìN^·'ËA¿éÙQ®¯'¿Ë	àØ·*"¿ëH©2øUNASNone?ïúßÓ âŸ?DËЪ…š?8¤Y:2R?;	"jògë?0]£·Iå?5¿¼ûf?ï'@?˜0ë7úv?‰›ØG±Û?ˆÝwÄü˜?Œ¡ñ>â?'ãïêcTœ?îՅò.z?'/Š×ë×?Í½Ö8¬?ƒ2>áÓZ?–hbúRk?‰BÒå¥?îí*ë'&?™Ö1´ßÄl?'ìL0e'•?"ŒÌ‹ò,§?˜ä|{W{?"ž
QŸª?ïúû¿‡?o.²Ã}Âõ?6f5N ?S"•Ü¾7?1»ÍÁšÕ?fË‹ã`Ö?ï©q2Š
?€Gñ½éK[?u?|:å¹k?n"ìãðä/?v»"wè
?v÷|ãPRñ?ïhÒì3M?ƒolòŒ?'¦œÌPéc?zÑI4Wš¤?ƒ$݆¸©E?zi9Š:?ïº5ÄÄ%ð?uiíÐò?sѸÔþ5¯?f*cú{Ë?n&Éÿ¬V?kÙ­øú'ÒAGN3FGL J0639.9+3250@fÁª:э&@(9äSÒÀ:
¬í#À;ˆðÔéÒÀw4x­Ç@6 \@ó@*·àŠ"¿ãÊ´p×ÐÙ¿æÍó3F‡¿é‡¤t>d¿ãžnÖRªUNASNone?ïê³ñšÈª?e(	!ÿf£?N	×n?P°¶`²6?[—[:‰?`æ¿Å°×V?î´Qä¬Åú?¯¥¬ÁLb›?uýuY›ï4?{à_t"_?¡û3
Æû?® òb	iÉ?î3jñ:•R?™6MXž2Î?':ÎV;€G?€´²ðœÑƒ?£«éĨ†´?"uˆŠ€?æåãÛ?…
Ö?3¾ì?$Wš= ?3ft[G?‹ˆö•:h?"ò\FÝN?ïøØo|÷?O\Xí"?7Ýà͜§d?Aà@´?@±
N#ô?FZ
ꅹ£?ïµ7pôM´?Šõ'"]Ì/?`C"Œ
1?oå
^­ø[?}B};´ì?†
—*Dc?ï\$GvÐÜ?{¼¸âS?€õ$Å?m""<Õù½?ˆâ©þ?tH"œÉ\§?ïëéã^Ê?\uU‰ÇM>æ#á`·dø>öÁS#:p?cÿøéÎIÖ?\jß<©
1AGN3FGL J0644.6+6035@ca…H©¼ý@6˜)à¤&À9¬Â7G"êÀ;߁SQ¶¬?­e±p›@eyþ§@63Ÿi½3¿ê…wßƶ¿à­¦t|¿àƒ¥p´À¿ÝŸôôÖx•UNASNone?ïí`^B34?`Ó*m¿† ?XžJûö3å?]Wƒ@Ï.?IAð¶µoc?F³0:C?ï'#BÞ*?'{/'³¯?x–_æå
Ì?z†k¿i?ƒ,+WÎÉ?ŽæÔó¨Qð?ïðÙÏó&?ˆ›{'K?ŠÆÿ2™"?€K˜ªzN?¾e'gÑ?{çþrQÐ?ïFŠñcZ?‰j[Èmç?o4}0
 ?g~•Í«EÉ?"H-_A€"?‡ Eޛ&C?ïù³ý•c÷?FH'
‡ÙÀ??C³o>ãQ?Aó´¸û±´?3`íƒa+?1i©ÞÄã?ïÕÏæîÈ0?sKøQ¹ôÁ?aQu½k5Ñ?W&áŠ+ä÷?hÞ£1pó?p7ŸÆ²Á?ïœCÎG1?w8GÒ?y)äÞj?t·jY¢?xÇC/.ˆ«?a´¾àD?ïÜäõ‹C?e"óÖS?T,ft+Ÿ?B™¬«%?i×6ÿaÈ?c%«6UK¿AGN3FGL J0647.6+0032@j€Îš,f¿ã"‰ÝŽæãÀ8›èPðÀ:ñ#±µð?ì­½Dõþ@.{ÏÚm@¨Ã ©-`¿ÚPâǜ'¿ê½"6± ¿çߕÒ9É¿âVxÄPÁ'UNASNone?æ2—#j
?ÅÒ[, šT?©Çª±Ánû?¤­Wþƒ˜?ÐÂ¥|%ëL?Åv´¸êþÍ?¥n8¯ÙRë?¯·ˆxý\?ÀÂê˜11?¶b4 ŧ§?ê¨kºÊR?¿;…ßtç€?ä[n°«?µÃÀ± ùê?¹È-|v.l?¡sy¾É¯?Ð×Õð2Q?³_"m¾R?ÜDc
«Œ?²_Ü£¶QV?½§ªWƪ8?±DŽô?ÜQ²_c<æ?³pcOÎ?ì'Ô2Ûÿ?»]+»Uè%?'šh3‹–Î?õ"'ÀF?ºZÄ`†lZ?º›—O]?ÀÛEû%¿?Ç+¿÷QZ¼?ÀŸ"[*.c?¯ëAæ;?çר¶ª÷?Ê+t ÄcÐ?ë¹8<KN¢?¥¿ [®D?¨>ÜÕE¦¯?"NÂ3UgÈ?¶ϳp«? ¼i¹R5?æGœ Ýp3?¥[w"™?·»ãëSHó?$ÜZØæ?˝†³»?¢é`·	MIXED3FGL J0647.8+1751@h'çÀn¹@˜Ôw¼À9Ži°ÂÀ;3è?ïÚ?óàÆ>hE@
»þ5¥~T@Ÿ\"¿ã†3é!ӿ죃äY9¿Ý<è7'¿äà劫6œUNASNone?ޏlp&ê·?Í>î™6ƒ†?µÒz~fÜZ?¶7C°{T×?Ûûôð#áS?Ì«ñÄíŸ?è1ø³ZŠæ?ËÈÿýj"?²‹7p`?´TJö'Q?Åò®&ª ?Å ^Ïï#?æ¯qÃDkr?°Ò'QVô?¿'ƒ‡«ÒÏ?¥ù†¾¯?Åx÷/hÏ?ªˆkEn?áštM.Üâ?À-¸»ÙñŠ?ÁÇsWÌ«Ñ?½÷«Xïìs?Óç]¹»ðS?ºŸéïTâ?éaG=VL¾?ÅëDZ&v?«\aEŠ|?­Z–'à?ãÊƞpª?ÁçÝÊKM?í	­¹æ?½-º7ô¸ú? s-ô)éü?¥èƒ+€ý»?®û4Z ?´2£ø?ë_áåà?¥R¿RPN?³xô©ÏÏ?ëþ0ìÛ?±Š"Hÿ—2?›	¯õ$¸?æò"žj–?³éð°=U?Æ)R<ksÊ?²‰4š­?¼¶–eú?¦@ѳ9ÉgAGN3FGL J0650.9+6524@bĆnCª@8s¸<òϖÀ:+gÔûoxÀ<µ¬õ–ðÀÛ²t†å@Ó,8Ã@R`E:¿ê£É²ªÑi¿ãd1_ô\^¿ãƒš"ÉÙ±¿ìH¹IY²›UNASNone?ï¬Y²£Ö´?ƒ¾ÎØÄ?t5Óãͳg?uƒÂö?uR«Zv˜?}n00ˆ¬·?ï'D(è›?"¹•H>9?ug"±vß?X£ñ›g?€ð;4\±?£_¨ø€\?íYL}d¸D?Ÿv¡{$?¥­Ç9j#?'[Šrè³f?¤ëŠeꭘ?"a-J&o?ï»
É'Œó?€ž£"Uÿ?C‰$—?TbJ×?€…/ct¶?€7Ïg˜S?ï«Ôª;Ó@?­?­ñ¾"h?m^DóëÅÄ?ˆxC2¯ª¨?{fˆ}n?«cÝÅÏtË?ïÝó"¡ëx?môÔâʬã?[²£OS»ñ?Vùßêξ?d3‹áÒ?gÛ¿¹`?ûÐ?ŽE»(¾Ü?—Âûܒ%?"ÝCbafP?'e'AeÄä?'[ÃQyF?ïõšÝÒ·?YTJòLý>ücd~ÔòX?s%šD5Æ?TZ`¬ÂÂ?XÝÜÔFVAGN3FGL J0657.6-4701@p
:æ…ÛÀ2|?>pÎÀ:`%wˆÍ™À;µ£@âH_?äɝ¶gcD@
!¨[Ô<-@ÄÌ>?î3¦p¿áù¬_ç>¿Æxä ªV¿ê
%Á8L«UNASNone?ïSÂ2ÑÒ?•\S2ź?†yTÁ?'º–Ü~ZI?t¦1ÊSÔ?s½b<†Q<?ë9«*ZO?¿rìAîH.?¯ ¨.Ac?¬ê%¹?¶¤—™L2W?·¡ÌCf¼?ì{ªmDs?¤°ÿyÊ[?±>Ùï?¡8s¾,Å?¦-5:›ó–?'ºh.-3?é7ú[Œ~å?¶ñ%P)_¶?®*âÓZ–¶?¨pöe·Ö?Õ]Þ
?}?³®'rš?ï°Cä=¢?xа¸î>?|oÑíș?}Ý:Ö²(-?g‰<NÄÄû?cŒ£qö›µ?íÎ`Q4·(?®0ÚDWéc?Ÿ@õøñí
?œ	¥0«¸c?£yñód÷?¤$1t­!?î*éhþ‹?œ-[Ln?£ÿ³Šµ$?˜ªãqhÚ?'¼»¶
¾f?ƒd«ÂcW?í:ÛÜñC`?žp?`Ɯæ?§Ï¾
:Œ0?"%♑?¤'"$ùoÔ?"ržRòÞ]AGN3FGL J0658.8+2318@hÈÞ*Ã"@'äË:%•¼À:`e)O…À;¾eÌ³mÀtóL¾J@lõvº@ZË`6¿è‹á··ß!¿çOY ˜&¿å©MIg…©¿°ã€("lUNASNone?ﻀá*ÁŽ?ƒQܧÇjô?SŠÛ_'"Î?UÍ@…l>?}\ؕzG'?'4à«}§?îïb ÍÚ?­9fr¬?rÒrH/æ@?{üÇ&Í?g÷f(?¬
 xù'?íèºÀS?šÿ̛§ûW?"´ø­–Ê´?ƒ¥¼óÕ?§×£‡²{?•ª©@¾|¡?ïÇ6ou%=?vÆ<°w'
>÷vÍø|"?\ƒy©?|MQ;'?v¿3J?ïï
²¿
$?b!É6…²?;÷p8‡?;Š*Œ ýw?Zì¾l'˜?`·"Žó¿Õ?ï¿LÀÍæ?'¿§ÄVeû?\PšV•Ôa?ZÖÑY`°Ð?yi²ð†|
?€çÖø!ŸÅ?ïI==D¦p?}$ñˆbI?'»¶'Ûm?l-pՌÕ?‹¯ôìÿÜ¿?vøËî'~?ï÷}ø±?E'"YG>>Éíϳ|­ƒ>ɪK,Ç¿%?P÷én¸¬D?EŠ9bÍÙ«AGN3FGL J0659.2-0439c@k>§æšÔ¿ÙWŒc¦¬À9-QîÊNÀ:ÙàU?Íu?ÖZãü>Ty@
Ïd9:‰>@3ÛËÍH¿å¯ÀCkSz¿åЬçef¿ägX6Lî¿çf.:ÙxUNASNone!?ÐlR¨]Eš?É>_°®wç?±Á=I"
?¹¡¶*–N?呯Șq?ËàTZ–(?±*4‰ñò%?º€Èè;¾?½œ8k'†f?³ìõíD ö?ê'2a&5Ÿ?Áíg¤ }›?âÁvr֔Õ?¶ïaÓ'Ür?¹õõÙ4Ä?£rãdxV?Óÿ•¥ éã?µ4ï ?Ù?Þë³a¾{?·ïÒcd©?¯–;–`û?š[å=Ó?Ý!…žˆ'?·Y~hQ'Y?á†F*(??Ò9\¨!œ³?§'£`iö?¼àO^¥
?ÚGÌzö?ю®w)à­?Å¥'VÃ|?ÎloZçéD?½sΌs
?ªÛ•Ér¨©?æè%˜À֟?ÎK÷¥='?êÑ`Ä÷ý?¨ÐPà¤7[?©"B~Ü}?"MÁϤµ°?¼éZÙâ¬T?¤ÿ±"šØÝ?æH}8K1=?®Œßçz°È?ªKÒ×ÌÜÇ?Œdԃ	H?Ð%‹3"î?«Üôl‹ßìMIXED3FGL J0700.6+3557@f™³=¯ø@1C'·þ	À:NGKîëÜÀ;Úa¶Ô=?åß*¯ø>@ÖшsW@9¾ Œ'u¿åˆ=^¸ÐŸ¿Ý°… à­!¿êð
-ð¿ïÿOÇF.UNASNone?늤(
W"?¼îé}î©}?ÀB(¢ä?¼Ã:…j–?‰4tv«u=?–‰©Պ?ؼîþ"n?Èäb¾nö?Þf¤œ#"?Ç0*àSg[?…V|ʒ?À<#Ï_?è–4	?°Úãîñ
?ÖxK"ýo?®E÷)Cz'?±]Ѧj&S?˜Ôg¢…äL?ÖaaË2T!?·Y†€£"?â*èfäÄ?»ðw?µ#5™|Ù¾?£Ý+SÓ­?íÚ#…ý@Ä?±H25ì§Ý?¯Šn)?°'ââñ~?z)év9aÝ?"q Å ?çéÈÑ?£.?ÁG´ù¶(µ?Æôc¿åU?¹'Ûš|	ê?²Éz°¨Ýb?²Øx¤ó{?뾿àDÂ?¥t^"âŠ?¹9¶ÂwÈß?£©|Âq ?¡ "s_¶-?ŠúÂ1£?çJ‰Í/Š?©À,`ž4æ?άʵ¹?©O³Êñk?¢è°;Ä|?'FgI.MIXED3FGL J0704.3-4828@p-xÔýó¶À1ô®…¹èÄÀ:áH2ŸÀ;Á™úèi¿ÐàF9Ó5@
¸ƒ«R?ÿ–Ÿ‹Á?äß5eù•>?Š9¼Ç?ÐƖ4èȉ¿éåH3ûUNASNone?ï­Ä;ƒ¹³?ƒóoñÐø?vuÀßIJN?xàšá¯Û?r¨!pçå?tj)_J?ëÔeru"?ûKc3^°?±äè¸RÑ»?¸^ØñéÔÕ?µlt‡u*?¶˜4È<M?íi)u€q?£X#ÙS6ì?¬ŸD®y³G? ·fÓÜ|?¢ú(º.E«?Ž<'Òä–?ì}ÙõH‹?µDù^Ý"^?—×qVß~¹?¥µƒjd??¶Sþ»Ï}?±"áÖ(©?ïÕlÓ?q?-©dÊ?bŠùi ?bˆóÁô¦?hoš"+˪?h"ý@€?íÁçf:?¶uϤ"SÍ?¡Ç	¡oN?«ºÉ¼@?¢(ÈmŽñ?¤O´¸ÍÊ?îv©'ÎY?˜~S$ç¬Q?Ÿ@Ç?"í	Óec?'ŽàáŠR?ƒ•ÈïŸ]?îîæâÀ?•Ï«Eà×=?…œg<V?'3ˆ"§§?—U4êâDU?áë"yy]AGN3FGL J0705.7-0006@jÕQ—¢H•@	Â?«ºÀ9ñ½V7D:À;Z³˜H`Â?êN¤d'•ˆ@ÛÛÐö¨@/² %ÏÈ?뗩Ás¿á0DZb–¬¿å·TѤ´¿ïÿ÷ç­£½UNASNone?á •CɃl?ґÿëÌÜ?Üpj¡3—?Ò¨—MäåG?šÆPÞt'
?¥õIvI;?жF-`áA?СH1–?̋i¢}eS?¿b­¸ú Ý?à'€&Å«?ÍÉðóâT7?ãÂ:w  ?´½2(âz?Ðó`­-(?²joëHó?Áš5Üìæ¯?§ú¦õƒÂp?ÞM/L§?¹Í¶¹‡m?Óæ[X<¿?»@$%ÍS?˙C˜í3?´O°‹ÉXk?ç±Wÿxú?Ðlô[BW$?ΚO¨p`?ÐÙp–m?•'í¿?¬¼Ôf‡ ?ß!B.<?Ô8ƒ9Zê‡?ÅíBЬwº?¼EWx>?ÕèHVŽŠ¥?Î}ui³è?ç—àà'6?¯Jµì±K?Æg·­|?©Ôêe"Ç?¶rōÞèh?£e—{µ˜?ç§E·¢Ì§?«FŒMΉ?Å–€,³?¨ h/tÇ?¸†¥B#£å?¢ùž/›óMIXED3FGL J0707.5-3111@nVúñ€À%V"uÀ9Ïi,êCÖÀ;"ëžI+ÃÀ‡¹-2¾@Z±ƒED@±ù`~šæ¿ækMÿm'¿é|áp®úæ¿ç«Ø)2…¿Ú•2c¡ÝWUNASNone	?ïiZëš(œ?ŽRö©w?aú
÷˜û?`aÿV¾Nï?•a1»g^?IÞ襒Ä?ï2·Ó'7?¦wšžñ*?sæmŽ¢w?‡¸üeŠ¬?"¯j2ÆS?¤J×fD2?í"‡è8°?›vv•7Ô?š².0­†?…ò!‰×H–?ªe0e¶X»?"
Ä''h?ïÆ)q,Vå?"=x­÷,>Ô6ÃY• ó>óýí«Sî•?|æ9Ú;%=?"<Z³í?ïǺ|J/?z€w¼Ö‡?NVðcۃ ?Iüqy˜³ó?xWãÞ5¦½?xÌ´ùB]à?ïªbÉ<¹3?–]ÅL¼ù?b­]6?uB"pÒÏë?€¼{y-ø?'ìó,ÑÉ?ï/x
W×W?~",ÇÝ~?…LIï23v?mÏP2	«?ŽÕ²³ø¾¹?uqÞᗠ?ïö§ôr¥†?T|«	¡>|ƒËìhf>£ÊŠ«ù˸?R¯¥O%qE?T|.ãs%AGN3FGL J0707.7-1035c@l|"µÜÆ¿óñ'©"áÀ9/%Ž/LÀ:žYò»?í†ý1é@ÚHtñp@ôCÀI0Ë?èÞKb©î¿çÐgõ¿êû\˜1e¿éª{"œ UNASNone ?Årm̝c9?á7ŒxÆ?Ӊ؞¶?Í=O°†3û?àÞx=ÔKò?ÐðSËÀCŽ?±¼…p±‡¼?½œì†Ùc?Çh¡QýV`?¿=ƒ"Ûªò?çîFýjyq?Åj!ba…<?ÓyŒ0nw?¶3ݾfÌ?Ïy¸³eG­?³ ,öL0?Üɗí³?µé1VÙ
t?Äâa²U/æ?³AŽÛC•Ó?ËÁ";d7Á?»+ی>x?ã×đ¦?¿EÛMæ_<?Ê$-D9sr?ÈØ»Hý5?ÍÛ(Uð³˜?Êð!2!?â*™uv>?ÐÇÄt–?ÅKÆ+aÇ_?É}¯iu˚?Çb9ŒyÜ¡?ºWAÅÈ Á?äԀ	?ÊÕM[lQ?âÑq¨C?¶(6Ñà?ĕ…‹£?h?©ã"¬¨f§?Ð[6ÝaÅ?²«HPæGS?ҘϓaØ?¶¹3¹š?È1¹0?¯ãÃ2Oð?্׳Iˆ?·Ê	:E´MIXED3FGL J0708.7+1747@hÙm›äÍu@'y»à~íÀ:d«Ï&CaÀ;·'ä™r,Àï a^ë@ÖúM8—÷?ýc8¢gI¿êD0¦2{ ¿è
¾Äî©c¿Èú‰ÏÞ5f¿¯P8ï—ÚUNASNone?ïùÊ]ÿ'?MŸr¹Ê0)?øMäø?5;û;RÁ?FWvNŒn?L·£[Y×?îþVùr-€?«¹Ïé
ªu?q¡[µ
k?{Ï5u–NÈ?›ÌÊýH£?ªÃ Ð°â*?îìO¯žFZ?''Xvqrõ?€ŽÅ[»{å?r.T‰<§Ã?š.§Vr\Ò?ægKê?ïê—b?a£cd+ã.>¸âìýgb>ˡ欺|‰?ee€ù"Êá?a¢hºž?ïýy¾Óæ?2þi(ðñ?IÜà?ÉĬ[‹?/ìµyŒÇn?1»yf*?ïÿ¯$h?'‰^ýS4Ö?ZKïÐYŠ?Y±¯ð0Ç?wé¤ i­?€Ê™¸Ã–p?ï"d{(¯?w×äð't@?sÕ­ Sw?lk…Ÿ^M?<(]jáð?pÒ+¾Å,*?ïüµ¡s=ö?0N×{F»
>¢gåü´è>£$uÁÿ=æ?:I¾Ã%Uc?0KÝ´e|€AGN3FGL J0712.2-3806@o0¼¾aÏÿÀ)0HZåÀ9ÚÊ÷àÀ;uÕ`EK?êUVß	æ3@Oþáqõf@5SÀqt·¿äÆ1ò/K·¿äŠ‹ÅN0î¿åƒ¾`£Xà¿ïÿȏGÓvUNASNone?íHRËe)â?´i[éÁÂ[?«ŸûÉ¿›?°:AšT*?Ÿµ®øüU¦?¡Ê¸Ým5?é\Þiú'ù?œÌ@­;¯?¶|]¶X[?°™?‰É;?¾POV]?¼<\tŸ¡?èòY嵸?³µž̶!?Ž¸ü«?®ð"]4,?³O¾Ù??ŸC‰ã0Jý?åü?ªv÷?®ó¢.öÙ?ÃB2…õ^"?©$‡ÆHÔN?ÄÌÎÎp"?¤¸ªš·•?î҂ý¬?¥n–v#¿?—ô9e`Þ»? .Œøyãl?‹wõý¤?×ž1åÈu?ímoX
ÄJ?±hÇë¤o?¡{¯ãWß­?š®×
Á¹™?§­Zž_¯?©9TŠpÜ·?í]þ1?ŸLÀ²ö?¬úTÍQ}?˜ãîÁ—?šKHÎU,?ˆÇñkž¦Í?ëˆ{üs?–x;+ùMÌ?¶`…¥³?'Œ³Xçµ¢?«G*äwg?
©&T~AGN3FGL J0714.7-3924@o^ {5À)dBÇû¬´À9æxT¥sÂÀ;e?åë€@
}ŸVœïº@œÀ? ª¿Ç/I=O…"¿èšÿ'_I¿ì¶yš†åž?Ê•—R+UNASNone?ì{vPX!?·ìQÃž?¬žy"6ÓÕ?°ÏoZÕj?«±/z{x?­†Î}w)?îmýù.n?´³}|P9?ˆ."›´?¡èŽÒÉč?¡ýžÙá?®{¤r,ñ?ëΎ»;¢?§âö‰þ?®¬#Ϋ
#?˜õ­Bx2‡?¸+y¤ˆjZ?¢¬wèzð?ì2°œ?':?´z¡Xk+?Šf¶Æºµ?šŒqaý5?»'ÎG˜'U?²á@òƒ:?ï-‹Ýˆ²?Ý҇
››?"1b¸+áø?zEA¸
?5Òüþ¨?"AOŒh?ï"ÞGã2Y?K1y8É?qd,¬†³D?…yªX1.?†W·\)?•ùŸ"Kƒ?î.Uï±åQ?"×}/_ý?œ)6¸€ñ?Œ[a!CvÁ?žüãjô?‰ÜTŽw?ï;Ùå±m?'ˆ—…ñ…º?oWF¤.fþ?xA_Ç.?"³ûçä͗?M,DÝGAGN3FGL J0716.0-4525@p
quŽÀ-âÏ d#–À:G8£µ|À;Á'²D‹JÀòõ¼Û5@
'1µY¾@åÔܑ¿ì;lÁnþ¿â2öà´¿åM‹\¦/e¿Ý"ÙgK#üUNASNone?ïÑãöÆ+¯?q"úâyÿ@?Xöµk>·Ö?\ƒó#ª}b?pÐW(­^£?k¦PËÅFä?ïx€Ë+G?"8¶É¸î?oô^µ
Äð?y«sÖMii?‰âµ†#	?Š>æqmé?íŠJŸiþ?›}3ö?œ¹'[²ƒJ?‹m8ËJ,#?¨þYÝP"?'r®1*‰?ï±Û{˜Z?~p´
ZPï?Qùԇ?ÞIJÌe?ƒtìÛôԜ?~bGm[ÞÝ?ïîâªý?Z곊UÙ?@-Êµó¦?A™÷÷sú?Z%\cRÀ?V'΄0ž?ïÔ®a8w?r¢FKžÐï?V1×xU[ç?V¡zÀÝ?pYmÕ©"?mí–XŠóF?ï"2´ªŽ?€¶…¾‹"?‡á¾«´¿´?uê±?'"&8?sƒÿÕÀíÃ?ïñz®ÇÔ?R'Ðzç\Ý>Ïä&í,¹>ا¾rd·?\ú°ÊµˆÊ?R~bÒÏBAGN3FGL J0718.9-5004@pUS÷ÎÙÀ0Vy_goÀ:¦ý/À;¡0-Å5)?ÈN‡Jj:@q¯åC;@"FÀXË¿äbîpFË'¿æeÔñ–¿Ü~;)vÆÜ¿íÊö´Ò°UNASNone?êÖÚÿâÆ+?Ái¿·:"Q?²õsÃ/åØ?³kqú\­?¶S´>•ÏÑ?¶ÐãôæÚ0?è
Œøî¶#?ÅӉ"鱊?½ç[aƒ0T?¸À
¼¸î?ÀâkƒJ?½Ïlò?êygì½ï?¨êšÄ
2=?¶i%º»'?ŸaY_qR?µËšßÊy?Ÿ&ßy?æœ1"Ö?³-óè3te?·j™%"Rý?©+d?ÉÙí¦ø°?®À»€ûç7?íëM:	U?¾`fr$àŠ?š†!¾!Ö?©øÉD©"?¤+N‹žò?¶¨—>?í1¼™+"?±H¦"¯÷?¡	
Ù}!x?ž
'1<ÛJ?¦Ö\>V?§¼–q6"?ínwÓ(å?˜ã¢ËHGª?¨u—CÄt?'yo«ÕŽ?  'Aœ²?‡/uKw?ìT±³ì?š‡NÔ©"?§Ðo×nà_?þ¥ƒ&?°""Šð?"æ¹ly¤AGN3FGL J0721.5-0221@kOuŽ!–S@c)ÞÛhÀ:Pc–¨M'À;YeΑÀ¼Š`Á‹Ñ@
›ÔeÈ[Ï@w í?é¶æà/'N¿Ü.Êz¯k
¿áÜu‡t0²¿Øú•aˆºUNASNone?ï´ø$?}'—¨¼?OÿŠ+ÿ}*?FàjìE?€ûE]8´Œ?|X0½gø?íwÈl"?¿ü\î~´w?~"âI?‡Û†¬Š•£?±+O¿˜G?¾$¶Ԉ?í·îȎéV?šÕ>¨Š·Ï?"ÁK˜›ê?'Õ™¥-'?ª mïØѤ?–ÅУ(á?ïN*?-—?ŽŒ¼öÇÆH?(ču¦¾?4uù»?–	/:i?Žkâö0¨§?ïå®S²­?j9ïŽ8ˆ?8>TÊü¼?33`ýí=?gIâ1Åî4?iAUÀ
è?±þ?—}ÞPx€?cÍOõzÜ»?k½•X¶ŠI?Š¥§ç1ŸW?•›8f_?ïÁÃuU?‰SŽdµ¡?"?"$üx?s9݈½Œ?'è6Œcc?…´ä†ym?ïۀ5çºÜ?fy(Êtcò>ötd[F>ú#Ø®?r)p¤F]•?foF»¤|AGN3FGL J0722.2-2648@n9XbNÀˈ¡ú'+À9œÝÖ³ÖÀ;R¡w´l"¿ðóaHDg@
ˆÝrâJ¸@œÁ¿êPGÕpy)¿àՎL"¿å!ÙJåÀ¿ëÊ}^œåÌUNASNone	?ã"ú[9?Ç'_$†¦?ÓD(ôjön?Æ-pu!ÙÞ?¶GŒ'~…?°Öi2†e?êc"¤ë?Åä1Úåá"?£x¡EmD?§2Ú_ï'?ÂÈI§¶4Q?ÂL)%Š z?ç⍯¼¬Õ?®?×oQÂ?ÂJF'à!q?¦Ì™IˆLO?¼W2ZVt?¡?‰¡·œÐ?ë @TƒåÓ?¬äcw¥|?Ž6xz?‹°T´×Ë?Á–ëDî,Õ?«ì"VŸ£?éØcƒqJ?À&ëçš-"?§£n?ßÐ?»ûýÅpÀ?§ÛA+YÐ?¥´gCîÞ?î:ÍQh9?®ã ì̬?‰Âž4XÙ'?›©!O?¥í‹œ÷_,?¨Sü{m
?ìm)èBn?¢

ÀŸý=?²N°bu?=«h@^©?¤Y5?A?ŽpÈýÑ?îz)¿?'«ey‰Z?fº—š€¿A?c:'A5ä?¦óž"Gx¤?'D-ëñaIAGN3FGL J0725.4-5007@p\å@ÌxêÀ.ɶ'!%À:¼šTª|@À;ØúËÙ,?í+žMÒ@x³yi£]?ÿ€@W3¿á,s©£…‰¿ïÿ·¯'C?ïûûU˜°2¿Þ«úõ—UNASNone?"èÛ?'ú¼pÊrž?Q-@‰?Wɱ6[Ã3?ˆ¹«bó*?'¥ÿØQ?;·Õß?²öc˜š"ë?Œç‰vÓ]? N¦ ûÿ?ŸûSʌ¾…?¬öjS'h?ì­¼­+-?¢¦SPe? ²Z"L£?œ >ŒHF?²8íÊd©?*(ÅŠ?í¹ïa;&?¹²:¥Bo;?wf²öéª?™}­Ð"IÒ?°ºÆïuì?¸ŸkÿM?³?ï¦J²ßC{?†&Ù¨?Oþh*Ɖ?P/ÆþƒKè?"ml»zJ
?…Wûêq£[?ï]nq¼tª?£t?l†?{ƒ«Þý?•RÞ-Ïy?ˆæ¡»û9	?•žCÉï¨?îGØݸh£?—N{…~Ñå?öpHã)Î?'ÄÀÖø´W?£:ãÇé?"‡èíê?ïgü¾'U?×‹E,ªº?J«–'£?"û8×Cï?"¶$Ë®˜?-<¥×þJAGN3FGL J0725.7-0550@kÂW§†Â'@ªÄ°ž™À:&¸©õÀ;']<9A?çâÉ|œnò@äJ¾À¶?ý›ù?ò^W?êIHQŽ¤.?¢U'Õ«~¿¼Rk¡}'¿à)êÚ©Ú/UNASNone?ïôe|L?U7f"}'?@Ñ}Ûο?:ÏXíI¿?NôëJà	b?QaÖ{K¡¦?ës-œùÓõ?ƝB¤Ø?™ïÖA^§Ó?¡¾#ôV?½ê†ýÏh?ÃòQÙ3?îJ"(){?—¨ãÂb&?H¼¾T?Dî˜ÕÔ?£2©_/F‡?"Þînz_?ìíÚ1Ø?©9Ë®ž÷?™£«ç$†?• dkLM?²(C>v?¥Ï02Ûq?ïùL<÷?Jwl[[m?1H±¤µ?+
?>?CF!kÜ?Fq7_¾Õ×?î—á+19¼?¯"šùYâ?ƒ§Ô#'?ˆÝcÌAÝQ?¡ºCYÝF6?©áóòÍß¿?ï:æ´6´?‡Nãö†šé?~ðNpÌ'?rçŕ+»è?ÇbºZâ?ƒ†<†J\È?îØÇ¿H)?‹Ñ1uݚ?'GŒßáw`?|ºû¯ßdS?'Ÿ{D"»?"éÃÀ™¶AGN3FGL J0725.8-3532@o`—ÌÀ"ôù;À À:zÑWv	À;qªt³0D?Ðx+úé@"9náŠ@ÞL€S¿éø$ÆLÄÄ¿æ7BÙ»À¿ãõr
É¿½céL&/UNASNone?鷺×NR?›\˜6Œì?s´t%¢?t'X\?™a14T?˜Éç¹8û‡?íIýQ7?»íðjÙ	>?'dxÜ|ñ'?¡úÿGðÅÖ?±VõN.ç?µß"2yf?ìÏ5üL}m? À8QƕR?Ÿ'§|À¡Å?‰œÄ"à?±¥¦<´'?šLmä+…Œ?ì‰d°XÍÌ?©˜{5¦6'?}ˆš/ûø?‡'Ç~¶À?¹äô…\?¨þ°Uºõô?ïÀV— '?€E®¤d?V"aø<Å?X†yc´K?z0#X|O?|Ž-4؃?ïôO•?§ã<ÙX?{j7þµWY?Ž7ÜÃÃlY?–èö)·?¡C,æÃ?ï¿'ûÀ€?Øeê87?‡跒gœ?q6œØëúr?"}™_—R2?yëUŒAõ?ï(tÓ3Ä?‡˜ü¯¡??jþƒ~|>3?h-¦ì:hÃ?—'•&2è·?…íFiñ¶;AGN3FGL J0725.8+0212@jÜÇ÷zö@@!U0H'ÄÀ9|DeNÀ;{àdYEì?Ä<fõÌ@õ½ê0àÉ@zDßØî¿å]àÛÍq¿â7ä¬M·¿âò|Ԛ¿ß8ÅJfUNASNone?ïÇ«ÒΑ?v}Óæ:?YJ0IL¼?Q#xõô=?wõ–5L?tNÇ7pÒ?íòHò.¨?²$`Z^?†ï"kð"™?ÎA€£µ?«ŒoD?¯ç[Oy=m?î9¾óE\?—ÿUyóз?"\i‹?ƒi¾?­HZ?¢\âąÖn?'·Ää`}?íÍÌÍ2?"YP>¶èî?€)Ø勔Ü?v|l×S—a?¯È­;3ž?"l£'!óH?ïòlŸ_?UÊ_†¹9?@³gÓ#U&?8䑌ƒè?RÎ*êí"È?RB&§ôÐ?ïl¨ûJ?–rElƧÅ?p:ä͵ƒ?q'\k×ú?ŒÚ㞜ùû?"f¥°¼?ïgñ6ʨ–?}†õÔ`EŒ?¢–C°&?q^ý×%Õ?†2gMš|=?r"}fï\?ïr¥¼	'"?tØ,/ú=?l"ë(‹Ç?T¶'UZ
?ŒMÖBY{M?s3Šb™N,AGN3FGL J0731.7-1914c@mRd"¿Æ·\"?ÅéÀ9©ÌíƒüÀ:ì±+†–ˆ?í{‡¬ ÷ @Ȭêˆõ@+ÿwD¿â%q/(rÌ¿í_ÇÑÃà¿ãöÛ¯yç¿×g£àeUNASNone!?Ղjd3?ÄôÃsV?M`Õ[¨O?…
Ž?CC?êV©â^{Ù?Ŝ%->°?¸Áˆsßÿ7?Ä©:²"£w?´O¡åkÊÁ?±"zބ?ê]Ú´Ÿ?Æђñ¾t?âÍ<µ=?·°×`Àf?·áѽ]ª;? Ç¿ÆϾ·?Ôm}>U?¶Ç™\<?ã?aÛ£e†?ºhhièZ?£:Xô"?¥‰Ì$¹ÑP?×øýµÖo?¹ò+gHä?՜ö5Pï²?Îîl•æ˜?}øöÐo,R?~‰ÎÚÄ°?äõ'÷œŒÇ?ÎaðU=D?Ë-qvԌy?Ó!-f"?µM9¢®®8?¨DmQÃëG?æŠünŋ?ÒîÉ2Ç?êÏ÷^=D{?©f¨Gâa?§¢ÁŽÒÕ?"Óy…"?½®äHXM8?¥×¡$¡?ê("~|²®?©± è
ž?£{õVœ?—5åτ?Â~°¿Ðåá?¨zÎQMIXED3FGL J0731.8-3010@n†!ê5"À˜¬}¡ìNÀ:|"}ÙI³À;ÛeìÃã¿Ö•´2Þ4å@ÆËG;¨Î?úµ1 6ç¿ïÿ(Ÿ˜??ïÿ#üY¾¿ÚÒÁb$Q2?ÇñÎ?yδUNASNone?ïÒó¤@ÖN?röƒ÷¾4{?Mci$÷?O˜xÍÀ>?rÙÀ¹`¹Ê?q?¢Ã"í?ëçíEb¤?È£H܊&?'Á¨ Ur? L;É­ÿ?¼P-"ã§Z?Æ>yH§tà?íÿûIaô?•ýÍúD5?'üAA"S?B'B€Œ¼?§F'&}›¡?'€Ø¡z
I?ïƒõñk^?‹õYP+Ñ?WòÞ;'Š¦?c®' "…Ì?Œ'ñ¥c?‹g»Í?ïçÉ»{E?cb*=Õqa?@tT^{´J?Aæì&
½?d/··Á•?aM¿5ÀmL?î—þcx1?¹ïÊq—Œ?{ž¦ rŽ®?ŠÜšàáK?£Jáܛ¥?·Ÿ¥S4{?ïsì?†ñ:àéžÆ?'­ÛK'ã?ršOJÃc?'ú"ܝ?'ü¶œ@á?ïä‹ÃAe?bÄ\Uh?7ËuËò+¾?3þVâoº?hzÍý—B?a‡Z¿vuAGN3FGL J0733.3+5904@c¿")³ú@<O…ô¡'À9ûçéóNÀ;ùŸ¸—‹¢?¹Q¥mü÷@=X´ÌûÇ@>2ÿ±¦¿ê
π8ï¿ë†ØÕÕÆ,¿Ó½ïù'j»¿èúÖ0´åUNASNone?ïþ'nÑ>e?"Ú²¿Ñô9?ÿƒ$Öò™?©#[Le?O`<å?‰™Êá‰?ï?~x´z?‹ÝBù•Pá?x>2Î¶?|0vuiAð?€‰?"X»¨ÅÙ?ïI"¬S±?ƒânI´ª?v.™,´|?lÒ7kaWö?'CÖg¬ìÆ?€òïçG9?˜nKb?†û$Úó­?`‡¦­ˆ¢?`L1n{u?‡ùµÃXËA?…·" Ho?ïÿKÞ÷?,*ÔK?"Ãzuߚ?K«;é^{?e3h—ø¢?Ý´ KäË?ï֋±"OA?oRU~8?b"
¢÷,š?Z¾Á‹:?fð@¾ºÒ?h#ˆxè|´?ïªf ?r~?u'¯¾HÎo?i?‰ì÷h?c—ܾþ÷ ?~,êÞÌyÏ?s,l‡¢'0?ïëqþ†??_\ï¤a?O'ZýŸH?@lô /M'?ZîªY8¸?Z«]ÍvÒAGN3FGL J0737.8-8245@rq3|™®'À9t_ZÙjjÀ:
jÿR[À;§£@âH_¿ü5V¹u,'@
Üme35Œ?þµˆ€»®¿Ì4Xþ…Þ¿æ×(Œ¼¿Òð[Ç빿Åkí4²uoUNASNone?ïٯѿOâ?y¶£ô†?1õÛnk£?;ÍrÐJª¿?r¹IN³Û?x«\ßïK?ïŽÁ
Xt?‹C1>L¨?iÜ•]?u!T1Z>?…ØšŽË°#?…Kiۜæ"?GúÚ@?ª>h¬¢ò?‹Sۇ@IÉ?w†8Ĩ? _ô¡ñåˆ?ŠG8³?ïŸPµ¢•?~f0­@>ó<å
ÀÚ+>þÞ¶/UR?ˆ"4H·ð?~¿¶§…	?ïë§E©­c?rTa~±Ò?.4|°?>›zÁXT|?bx8€æù?pò‰¯??ïٔwà{?lʽ8ê1)?Sö^u:?Ruž³ûí¼?lpXý¥X?fhYM«±Ù?ïc9úˆÙ?y~œyY†?}«ŸËÍÌd?iAá–P?ˆe¡'×û¡?t6ÛÉ;á?ïëAy?R»Ž}.Š>ÚhË"19F>×JbÒû—?a`³>ã?R¶
«7 ]AGN3FGL J0739.8+1312@iÊsÕº²@0Ÿ(bõ˜žÀ:+ÈbÚÀ«À;µ¢4rÎ?ôT&£,ëF@¶½[À›@àpÍ¥»¿ãGÀ-#œ	¿é+œÔóž¿ïÿÁÄ[D¿á<ƒbê·UNASNone?îg9£Bmk?°?_i_$?™Kj>Kæ?£ƒúylù4?™Í¹4S>¢?¦k¯ú¤¹m?ëÀΨÞÊÀ?ÇøXVXQP?²Ž#d=;?¼';'Žs²?®ÖΫº§ˆ?»¡ñÂO›I?é&üF?¬Q"$ ¦Ý?¾
€!"w?¥xV†}Ô?¹¬'Ìß?¡JvIG?߇áÐü?Èâ¥,°ô:?×îFI¡?ÍÄ,yI†Ë?Âd#§5J?¶'‰ˆò…Ù?ï>¢›²â?¡Ñ*"#?ŠEÅèõ$ï?•ÕYer²?†";¶®`?"ތø<?䂩œ?µ‡,QÕ?—Þ°ÖËI?¦œz‹Á§›?–K²'K"?©û"öǝ
?ëâªÔ¡ÏÀ?¤k(Bï\Ò?³:A¾h?žÙn_ä?«ÆÞ4Ø?—gþ%'2c?è=ÄHfB¢?º´åm‹&m?ÊðuڈÞ?ºLãwMV?¤ù¥¡Nj?—H¥lRçîAGN3FGL J0740.6-5230@p'DЩ*À,…æÿ}úÀ9ՓW`9&À;k¶1€¿ù‹·Shݺ@õÔȧÏ@×ß?k$ç¿èÄéeM¦k¿ßÙØ
e,¿æÊ^Eäv¿ØŠ—È<UNASNone?îYX¸ö"©?«‹!'?^?w×Þr?yD?|;"¸±ÈG?§ox¢—ÞÈ?ªÀÙu7ö£?ï;Û£ÝÈÑ?(zme{]?vy؟ÆÝ?'IùÜmZ?'æb¿Ý?˜['À`Ä?ìuƲƸ?¥äŽ¢x?£eêd"'Š?'sރŠb?²žÕ>qø? <9·ÉÀ?î̚e¤þ?"¿Ô~¸eä?FeÛh¤#?O)aÓÝ%?¢ÜÅXÞ?E?"›"È3ñ?ï4x'ª?"½­]lò?b¯<¥?ig[ã?‡qöCè?"™<ì3^@?ïÆ6´á¸[?|óJ"šnU?\Œ.SOàI?`Ô›í'%?uÁš=–H?w;åy¹Y?îî†
Ï?†øm©?˜¶?ŒôʉÿÝ@?xÜÜ`…·?"Á©ô~Ä6?~Ù'+?ッañ¦e?nCeãè$ö?@¢jJ7?>2hnG¾?€c¦NýùÉ?n#=:&Ñ(AGN3FGL J0742.7-3110@nÆw[0À®S<½öpÀ9{lØÀ;Ød°ƒÁÀ0tY™#}@¯h¸Ñ@½üÂØØ¿à±s39¤x¿èê|ã!ð7¿ä¥ïÑ3º¿íŒì"Š³oUNASNone?ä nêÏh?Ä[—^§?Åï£Þ¹V?¿ÛuM‰÷?ÊnT¯¸G?¿"K*1-?ë¹—ÕŽ?ƟtWiô?–v.Pè~?œÉÂ÷Ì?Á*Vº:½°?Äށh}öY?åéþG:Ÿ?±ç,:ÂI?ĔԅJN¥?¨þ'R
Ä?ÃÆ냾ˆ^?§ˆ2<]ìT?ëœÌáE?µªŒ´ÛsÂ?bÒoª,â?oþ•g×?ÁDqôäîØ?µ¡ë¬ô°»?èÀ¹½ÊË?À~"T$3U?¿Ø«ç7?º(Ö/nz?º!‡º¡s?±ß*aARJ?î)ʀ[ø?·5Ӯͺ1?"i¥ªXâz?ªC'X+Ý?¨Hî'ašc?³Þ›F	ñ?êìäè«U?§Á¡sÎF?·Ôj³6ªŠ? ßüTz?°Än	)É?˜D"b/æq?îw@Mokë?žcÐ0š×¦?2d•^'#ð?D:]òŽE}?¨g1úddÍ?žWÐÔ÷Ç*AGN3FGL J0744.3+1715@i\í(Œç@3?¿¤Æ†À:0áþ99À;¼RÀ—4e?ìÝ$ݞÅí@šö†M@ៗµi¿ÓÝz:iïn¿âkዲ¿ê—Ž$"¿çAê%DªUNASNone?íNL¶‰`ß?·ãš½?³èerŠ0ý?·{"þ?zSMšëÌ?x§Djy®µ?ç~gXB¦?͂ƒæ²"«?ÇW«3[2g?ÅëÑèÉ
S?µ]nÓVۂ?½5V}Tz?ëp`(t¥?¦âm•®?´¯bõü? øEu¥Õ"?¯›8}r«?—?`÷Øn?ØÇ»ÜË®¦?¾nʖš>c?ÝÄ+Á­gŠ?ó~ùkw"?Âè0Ã
Ó ?°µb
klm?ïPBå˜m? b®ýÓw?'.Ö_Ñ)†?ŸrSHkBˆ?nG>MX¦r?hžZ"Õ?í,Ay>|µ?¾µžŒ6ss?«Ï`ƒ?²ñéK¡g?¡l‡êNû¬?°Þa}Q'?íÿ:Åùžè?˜=§au"@?¢Ïs{d߯?'C[f±y…?šyÀO)͞?‡Bùo…-ƒ?捈Ӓ}Š?°Gç|ÿė?Ά¨ƒÊØß?¯Œ"궠C?­з¬ÃÝ?"§þDíMIXED3FGL J0746.4-0225@k¯\(õÃ@&*¯È°À9¦´%6nÀ;'ø
h9¿Ç*G@C¬@]XXܐ@Eß³.k¿ã¦H®¼ä¿Þý´7÷àn¿àjê.÷(¿Ôá)E\UNASNone?ïà•½¨'ã?e¯<"Çм?P³ÛQtÔ?I¯W¤2K?gTq~jè?b_¨†ÅJ-?îù•"X??¢MªÓ@?wÁ¤–Ê÷¨?|'Nˆ*†¾?šÜäw,j? Š×†zˆ%?îÙ¯^Û`A?NÃq)D?‰×½"?}y&˜¬Dþ?—ÞjÑ
?‡‡éÜ?ï91X"çó?"u‡–ŒÉÒ?R`
40?QHô:¤ì‰?—³Ô@O£?"09±
$?ïöQ`3¶?N3³¨®(?5¢\¸ƒ¡h?/Ú8Å2
?JíŒ;É·?I'ûJç…Õ?ï³r Rè¨?ƒÏîÁôi?aç3Y4€æ?]|Y8ö­?}S´Ûì?¼BØÄ?ï‹v"¨G?wîNl<›¿?x³uú·M€?pü°Mâ¼?€È¾ÝºGœ?l[•òýp?ïÖ$L:–)?aKEŽ­"è?>Ž±ä­?/-ë‰E"?sîßî¨ð?`¥1fûÖAGN3FGL J0747.4-0734@lF`ªdÂø@!£Ð|"µÝÀ9û™
þ`ÄÀ;wÖ	Œp¼?Ùý%	NÞ@fñ/
@笿'%¿ì+£3:Ê?©¸Á"bçº¿à›ƒ†²·"¿åë!²¾iïUNASNone?ïs}CUGä?–{ç-Ödí?qߨÉñ§?tÉTœ‹M¾?Š˜?d_t1?"ÿ¢ë…?éõ	îÛ`?Å$'Ïö¢ß?¯We–­	?­ËŒÜÇÂ?ÀUþÞ±•~?À¬
®ôcƒ?íVŸaA? Ý×a%^ß?™œFÔgj?‡9Í÷²8(?­ÐcÈ{0?œg†Þ?èœä£ibU?¯ÝÈe½|«?½5£ƒ…å?¦z¿Y‰Ã•?½{¥A1gp?©a¢š9˪?ïÕyMb£'?ƒ€~í%DÏ?RÖhiR{?a
Às.=.?p¿F(µ?€ôä/ÍG¦?û0…?²êàb²?•žµÀÊ>?š),BTî'?¤xǸŽ?«L)4'êå?î™deQ¶?—òáyü%?ˆý'õV?€'JE–ˆ¨? 0E2³2Q?–}ÍK§è?íçô4^›?–(FÌìM?«"ff_c?5'jiZ?£­W~é?Œjú›§îAGN3FGL J0747.5-4927@plçl‹C–À'ÎÛ0sÀ9ÛS¸
øçÀ;k(zrŒå¿Ð=tÄfæƒ@
pó'ß@B@0þ'î¿ç$
Ù©Ì¿ènè\ ¿ÓÞ d×ú¿Ý¨-óòðUNASNone?ï>űI?•o¶ŽubÓ?\4#'f'‡?\ÎöƒŽš?–d å±?"¹þxrUÔ?îáó;1À~? :‡ŸÍäp?~<|³³äÝ?'U(¶®?œ2ys
C
?œF&p{>ð?ì岐>/?£'"tÜZ?›6ïŽk¢?‡épüªPš?²
6‡‹"?žøÍÁeR?햯r°?œ¯Dçë«?\'³gö‡?`0Pút?²Ø?òVl?œbëTÓX?ïÍ¢Vë¡?{vêÂRÊ?H[L|uý?JÕt<¬¯	?vÉqÈú?yoš¶/í{?ïšÖº%D!?ƒÑl>û'ÿ?hw¶³™j?far]vü?ƒG3áI[?€0¨ßž?ïÈ0ìî?ƒã¾øl?ƒüèö²z?o(G@_,h?'ˆ…cñZå?~ÂY{!V?ïa¹Ð4¥?y¢Š])dr?UµF^aFÛ?E—",Êë?'mq½·V?xÈx?gçAGN3FGL J0748.7-5116@pˆ¥ÃÞç'À)1!îgQHÀ9Ê´øš°ñÀ;cÛêw¿¿áiô/3Á›@
ìŸÊ5BØ@÷L_ª	©¿Ù²öcm^¿ïs5Hم?ԡȕc1±¿æÇ"µ¦Y_UNASNone?ïk±"¢ó?–#.—èËx?K¢–¢wf?P'¸øÈ?'¬Çjþ†?•Ð벙"q?îöoïáê?¨™ëø+ãB?‹üAi_Ë?‡Š&§?™OUÊ?¥£OAÚ?ì	á%|ïÈ?¤='™,IP?žî6œ!ÈÍ?‰äyÖt…'?·õi+Æ5?¢1=óR3?íµ'±~E^?±0+,XÂ?JïÊ96»?^ªžQÓÏ?²
ÞfŽf?°ÿÁùöV?ï¢=u½'"?‰t`ä—%?=bËÅ:¨Z?>ÍÑ¡t7?†…Œ.g•'?Až{˜·"?廙¾³Pò?'«ô48Ð?fõšgý9?e60öh4?CS¤³LJ?~lTsi?î=ûÈ°)ö?™,Æh¡Ø?ˆpY ±'?{HdmG?¦-+õ5Ó?˜†¤Xì?ï{^BA?Š"ÆÝ#Ðø?I/t\…k?MìMôt?Œ±(×d«?‰¼ãÿ!yAGN3FGL J0748.8-2208@máî¢
?ý¸Ž¼ÆÅLÀ9z
>GclÀ;0¿ö$µ¿ÜÞQêƒl@
q†,ÕK!@ìÝÀ$5¿è»q§{ô1¿é
!þÑ$¿Ø'ç5¦"¿ç†Ú6(UNASNone?ìiz«Óê	?½åt›TÒ?	&Òú#Í?'•I÷ǁœ?¸±àëÆ?È?¼U뫇?ÒrA·–•ê?Óäb…†<E?°U,´"¦?¬Îjææ™÷?ä¼9¢k­×?Ó&Õ)Æ*¥?éø~P­?¬ù̗q?©û€_ï?"í©Oô?ÁÜÈé_Í?¨ÌuAû—?êŽä""¢?®û¹•Õ˜7?z}ÍÇás?s¯V7KÉ?Äð?·a<?®»4ƒo€?ï*žIè½?¢ìÂ5ç?yÒ¼o™UP?†¹z‡ü?"9x)÷?ž·‹¢)ù?Û¶.3ÞÉ?×À}oR¯a?°†ÿ˜Ñó}?«›'ªyA´?àó;û?Õ¡­fwz­?î·Ä/¢ã?•–Túž»?"@¯«YŒ?ƒj2U^û?£ô,=CÙÿ?ä-~¢Ï!?î)ÜcSóƒ?'m£:ðd?q>J«"Y•?_ŒëH«oü?«:pwãñ"?'·ÇfQMIXED3FGL J0749.0+4459@eÇ;÷'j@<ž†"ÄPÀ9áÀ¾¡ßÀ;âïÙAOV¿æ ž†~@KÃ Ô ~@ùY_í¦a¿æîÜü'.¹¿â^Ø܋ÂÓ¿â&(¦I€¿ëBýùóÿõUNASNone?ïéÖv]™?c‰{^Yq?aŒC'm"Í?a	ŸåÝż?E"˜YÅNJ?D]֑?ïN<Îè?‹ªÔÅã¦7?wò‡ž{Êá?y¾©»©"ž?€Ãèžvº}?…ø‡Ýö?îêlÝùÅÔ?Žî–熹"?"ÁWΞ>?ˆÇ5·y?âàâÞ{?}Ð:#-?ï…>QZ¡È?'tÙÌ ?diL"$%?a‹Ýõ?‰–‡jªß?€Ùi	Ÿˆ?ïóoZD³Ó?]OCí
1³?Tж¸­ü?[]ñwyý©?1BRØæpÃ?/ºßm׏&?ïØb©å¹z?nbæt&º?aÓÀè+8?ViËàÀ–?f—'Wþ'ž?há¢	¾9s?ï}‡²¼U[?}*KÍò³Z?ƒº—ÿ-Lµ?w¦¿ar=b?yÆö¸`Ð?h..KuÔØ?ïꎫBÓ(?]Ý[ïβ;?=Û¡Ôz~W?7¦$»›B?aµà½" '?\cIЪd/AGN3FGL J0749.5+1320@iç×Ûôˆ@2Ññ{ؾsÀ9ñªÖÿµÀ;Ÿ»@³Nw?éÀž‡§ @ºd>@þ–Ÿ¿"•¿í¿úÙ{?¢Þ,1¿æãtS¹æk¿èfžàs¯UNASNone?ïx^²4h?jvèQE?B,¶œ}²?—XV^?bØîY<™Ó?_Ï'ÂÕ
Ì?ë"i¹­
e?½-0îÖ?´0Yb;5?­­S‡Qô?®X²4`P?´ÆqJ:Ï?íïNÖÁ‡
?˜ÿVl0Ef?¢
FÕÒZ?'ÜAE*è?Ø"ü«?ˆ'—Aw?åQ6Ï}‰Ì?µ^¸Tí.?Ðú{àåÍ>?µD"Ò'Ï?±ŒYÿ2¢*?¢'Ö¾%0?ïáVÊ+÷?mŽîÒ^?h;¹cì=?k7W Í{Ü?I¹RyŠš/?Dkô?îŠi•šÜ?§Á
	ªƒ	?™``¶û´?•«L'Œ?•^2xYî? ¤±-gŸÕ?ïÁ?Œ8?‰¼>™Ÿ¢?¨-.'˜?…°Bú!§?‡?UÃevÑ?w¡…•~s?ì;"%éô?L¦À¬Tž?¸'ó]n'?™¶/‹å¥,?–Qbٝ5?†Íâ¸8ÅAGN3FGL J0751.7-2944@n½ºˆ&ª¿÷‹?cÃÀ9u°}á­/À;Ù|¸[¿Í_:û ¾@¦H<Ú¦Õ@šÿà iB¿ÚÎmÝdZÚ¿énÞov¿ïÿç
)"f?ïþ¹ç܌UNASNone?ï
cJÊv?£[Q÷~?…= T°Ç¹?ŽKâ'(ô?"ChÞ±i?Ÿ²£"PÚ0?ÔAÕh8	?ÖîCà) ã?¨¼I"Üïr?­›kS "?äS¸ƒ˜%?Ö°¼ÓF?êÖUؤò?§é-œœñ?©ìBŽõ?–å}¡*,…?¼W6|ö?¢ôUǚ¤U?率dõÎ? Ø2éXÁ?/³MАwA?MšlOêS€?œ+¥ò®¸Ú? Ô` ôc·?ïµqÅ{Zû? -d"glñ?d|Q~/­X?~>ÐD¾-?{ôzK¯±?œMìÕ:ö?ßNœÏÈÄn?ÙzôGºÿ›?¨éÎÈg?«d…¿áƞ?ݔ)VªJ†?׊ÿå[˜?íÙîsð?™AbUG ¢?˜kˆVÚØ?‡¾¹ÉÜV?¦9½=·˜?"Ý®7ð8?ïá[Ø"?rŒÛy>ü3:A"ØØ?Xú\èOü?nkÁ.‡÷Œ?rãŠHÆMIXED3FGL J0752.6-1629@mSýÉÄڐ@ôë?{@À9ÍRÿ" À;~%AØèd?ÝâDæ@
꟏&y@˜ÿ•!¿æÜ3"yl¿Ú ÎçG¿âm¡UrÅ¿çj;Çù ¸UNASNone?íä¶cC‹?¨éM3€G?‹k6µ[²?‹žHLlaŸ?ªÙÝŽ^?¦Ò¥Î¸¹?觷«—6Ø?ÈÄ:ênô?­l}íŠ?®žEPÇ6Ä?ÆÕJÓA?Ä0Ùÿ1ÆC?쭅âW£€?¢&aÎ*G?¡|"¼occ?ŒÆ	-3?±Õ‡åpÒ?›Ìúd͙'?èªçnÛø0?¥•56çŸk?µyNŸ?ž2í"ñÚ?—Ó[ÿ?¡EK‰wTÏ?éä4È?Šõ'Jîû?iœbmÓ®?l'×Õ}Ä&?…åž]C?‡8æDzÕÊ?í˜ÂxØP[?·élçÊ?"ÊRïȳ?›»òVk"ï?¬®ø9ú?±âZß#Û_?ï‡kD?…³''ɤW?‡Ã,ðXU?sÀ&>4Æj?"
•'^?×=ۂ0?íGçÌ=Áé?Œ«ÞMzGŸ?¤½®=¨?þß'pö?¦Ä¬u£Í?"íV&ŸžcAGN3FGL J0755.2-2633@ns-8Go*?ë©÷À9.wAýÀ;.ˆcp'?â)¾Fïu@(ä±ÅàJ@ÕÍØã\¿åÕIJ̬ì¿ç¯ ùN#é¿ë°ƒëÔÇ¿å['²ãÉUNASNone?îC­E"*?¨W¥n;?˜ÖF[?›u¸k!Ö?Ÿù"x»¢?ŸÆ0KX`B?´ãêåUs"?½wØib?·of›ê"?®ú\[c?êu•â?ÂAþ+ƒUN?ë?9âW$?¦Æ•ÊnX?ª[žpÊÁ¥?•"6ܟ£€?¸Øa´¯?¡‡D=­Æ³?æmZVÁ5s?®w,¶†(<?³ý"¦¨‰?¦îFò'5 ?ÌKÍ#ðÜ2?«:¿™ˆ|¼?ïŸ_T,É?†D—cIC?uÃë7«á?w2 ‹õ?zŒj¥DŽ?{MdmƒQ?Ê0؀ñ=V?ЏˆvåO?¸w‡P¢Ì÷?¦—Ää¶?ædØõؒ[?ÐǙâÏ?î± æ-á?˜ÜZÇê?—©ýƒ½©?ˆÿV‡­?¢"ñ#u#?ô%‰ÚèL?ì˜Ð±çKÝ?"ÅöÐɊ? øãĦÃ?…u*B`?²½"´¸?'m\QSMIXED3FGL J0757.5-0536@l6BB…@'õŒÒ
ú/À9Á‡ŸœÀ;•úœé°2?ð»¼x@dV7o-	@LÀM£¿äECÃ'º¿él~_½'¿ìf;}{ù¿ïÿhÅ*/îUNASNone?æ,,ÑÌ?È(—̘}?ÅùÐRµ¦ã?ÃF~ȬN?Á‰~úï?½8rbH¨?Á¢É Î_R?Âd¸¤ªLx?åç'°x?Æ{³táÿ9?Ê)šB¶ÞÏ?˜´tïÊ?åa*ßo?±Î]w}°?ɍr†|¨¿?¬
^Fä?ÂQÑ_ل?¤â›411'?Ã8>Õþ¤¶?­
é~c|?ç_LïFõ2?¸]Fš'ºØ?¾•ÙË
?¬ó·•™î?èc×
vß?Çõƒî?@æ?Äì9ôfe?ÆEÆÚ;î?³Ó­ƒ9?±"Zžê¸Ü?քT&↷?ɕæI<=?Þ³ßVø?Æ«
Ïa?ő!ñƒ$?¾•ÅQ$Ø?ê*÷BOù?¨2fŠœ¨L?½½‡×ǟ?¡þSÒkñ`?°ê¾Ñd.?—cKa¤Ì?Úxss?°¿GWQV?àžJq¤nE?²n¬E*Çù?²ëʧ6Bæ?œ¡rPáaMIXED3FGL J0800.6-4806@pk"¦óõÀ"·öµšÀ9¤ØDЩÀ;^
œ;4‰¿æu«'	@fÚÄT®@|ž_Ñ÷¯¿êˆ5Nt	ñ¿æ"Hô‹¿èb"ˆª"¿ïÿ˜ÞL•ÊUNASNone	?O!¬?ˆÙ²Ž]%u?~Š¤5`Sb?m³Øü-R?€Qš1Ýe?{$z†¢}?ëåŒrzØ?¢]Íæ}M?¢9/B*x?¥w×Ø萭?½ä;úé&?¾šÖ¡Èù?ë®BÚ+kO?¦Ó²Y®òò?²ùòAµÞÈ?–}ŠŽF§?¯'í×I؅?˜¬3eA?ê÷4¤øGz?«*qšVjá?šaäÎ*­Ä?–Xí;‰?ÀÖðҐ† ?¨Ù¤wsH?︵%:Í?|­Ò"—')?s¾Y:>Ï?t"iv†-"?oÎÜÿe•?hWc6V¹U?îgîÅß·z?«Ù«hµ1?‰J*dIû?ŒvþYϹ˜?£.‰PÞ?¥sÃSù½¡?îú–'0Í?"àNö€$?¢î'jœ
å?Ž{XTš?—"^SZ`˜?ƒ.éÙÂ8}?îçÍóØ?'¼0½û?t{"õa…E?pH÷Ԅ‰?¤b¨ZS?ô¯ayAGN3FGL J0802.3-5610@pÞ䣃'gÀ*YÛ©¢fÀ9ÏCŸ'À;w|ÚQ?ô —•Ž•@VϺ½Ö@í a´Ñ¿æ]†,n6Ù¿â:½h€Çç¿ë–‹¥|§¿îÝЮaZlUNASNone?µð5Úé?´Ês`õ¹*?ë¨j8>F?½"ô"Å}?©˜ðÊ€ï?«_ƒPŽÖ?©AžP¥™^?±U¦ëº"?ç¹H1
ÿ?Ái%~"°?ÊË_J¤z/?À/7"'?Õ-W½–ñ?µ­"™Ö:?àAx˜¡{?·x›''C|?ğošJL2?ª'ŒaÍ¥e?¿ÃþO¯H?¨Õ<üª?èrAUà²2?´üôᕑ	?¼Ð1VöB"?«]*€ñ§Ú?ÄuuuÖy|?¿×Žhyç?éšÃ´¹õI?ÂÈT9Šˆ?¤}îÛN÷ˆ?¡ér8Á?ÀÞ8(Xº?ºÀ˜Ðµ©^?å±frƒ]Ì?ÀªßØe?È\./¤n›?º×ƒV4?ã3ô¯r|}?³‹øƒœ?Óh'ô28Ú?±Tweu?¸¿º²Y^4? {ò@"?ÖÂ;ƒd?®¿= ¤?á÷'³Šö-?±\0`"³?µ;
K(4Œ?Ÿkã´*pMIXED3FGL J0802.3-0941@l½XdE#ö@%òéhSÀ9ŸúE«Û»À;ŽŸ±m¿ð·¹Ù&w@¤gÕ&b•@A¦`|l¿äÅMíHÃ=¿âøœ×Å+÷¿àРÖÇû¿ß×çõ"ŽUNASNone?íGÝ'{ú?²Ÿ¢E"?"ÇMã¶éÏ?"VÐ¬²?°ÏC‰ª~½?° 	?îzŲÀ÷?¶"#Õ§yÈ?ˆ¼M'sÏI?•ÒuĂoi?©©@=£GÅ?³Ü(ý}®Q?ìY5ïXÆs?¥tžY]ï?¢1_ˆü"d?e¥õh9Š?´ ¿´¶? "1€ëÐ?í¶ñđ?ž"¿ÿ¯¯"?hæw¯ê?f揯§w?±#ãÁý?ìý–Y£S?ïvùß)›°?–^Œú»!É?q]IU¸/
?wјmÝnª?‰'ã–²w?']ã¯è;?ï"í/mÖÈ?"ž+'4È?n'z›¼.{?t›Úè̎5?‡:Õz+¦]?$ƈåí/?îñ–¸¨?‡ÿ¥&21?‰ûŠš!>?wΫ´Ð2?"ÞH-òK?€Í ­>¯?ï}ÝeÿÂ?x²¦­0?EßþuPK?;Ɖt¨(?=È¿JMï?x<±~¢#AGN3FGL J0810.5-5214@p±´êJŒÀ$L`Ÿ±À9NeÜÓ«
À;E"äE?Ù¹e'è
Ò@\¬ 7@f"_ ¤{¿æÃǞ`¿êÖ!"VˆÅ¿Ý•ôgµ4Ä¿çø¡¨ör§UNASNone?í?zç|Ñb?ÁÊØ°°?w)NîӚ`?…±Coƀe?´'"Õç&
?ÁAó†[4•?ëzíè.Ô?ÁïÝäÞL¸?¢'K'2?¤l²ðR™ó?»$O™ßÿH?¼Ù°Òãù?ìe0¤k7d?¤ÏØG?™"CgVýó?†Š‡—‰U?¶êˆS`?¢Wè§ÒJ?è¥
~¦?°†™,yj?žÛuDQÎ?'±¶ÿ'˜?Ìý!~Tð?®™®ª\f\?éèiˆ¯¼q?ÓíÉIé
Ï?ÃÅRŠ/|?¦]S‰"1ä?ƂˆôRD?Ò´±'ß–(?îKW¤#,Í?°QúlVæ"?ª‡l_=—?"
¥EUfè?£ßãà!®Ë?¨»ïôˆí>?îÓiîuù?}ß,_N?ƒ"ÝPÈ¥?rlšÌ	Yv?›ÐS¡‰?Œ´ÏÛ_?í
ÉÇQ?–+{‰È?–—wܳß?|æˆfÎ?±ëéëP!?"È¢Œ*AGN3FGL J0813.5-0356@lG
Ø/×^@0C#À:ZPÀ;µ©FµÆ÷?æ4ô9´h@ÁìóˆÎE?ú¬_©÷¿ïû^Õ¸?ï­Z®CÂ?•ÉæÁ7¿ÖIWé9ÚUNASNone?ïæ¦iX"?†,ÜP$:?L{­|'•Ï?W­?uÚb?b;htÛb?…ÝœÄ?Œ<?î¡9ŽÊ'<?©'	?«v›s×?–¥VLyž?›-@³'©?£J•ÿŸ÷›?î"Ø=T…z?"ÝïÓÅ·?à"Vž9?ƒ"øžžþi?"®«Ø0?ŽënÜ(JÒ?îpM3Ô2?¦ä¨";êE?ŸïX™È^@?¡ɺ$§Ë?œ¢Ä䅂?œSÍ.1ñ´?ïê	&Lùa?‰Ôz+šV'?7¸±|"C?;~0²å?bÿêô9À?‰Èr.¢~?ï—
 ÂØ­?ó­ÔgŠy?u‹¿Ìi<?…
&?F÷<?~í#ÛW¤4?…Êp[o­Ü?ï6x#A‡?ˆ‹"HÚX^?"Ÿ	Γ?|ÞMšëèÂ?ÂíVÙKM?ƒ4.]~?ïk—Âm½?Ž¥ûIIæ?•Š1΂z0?‰
"^O?{¡lò}¨¦?xpN1¿RTAGN3FGL J0816.1-5044@p¤´êJŒÀ!9¨Íê>À9«aB:7À;#þT.U~?ôŸY÷î
º@=FŸ¡›q@òÙ æ[¿á‰3hH¿çNM;®=&¿é
ÂØŒ[¿í'íõUFUNASNone?Á-N%ì'?¸Õœ+Ô¡?á«úϤ?È­PI­H?Ô6ø~p7?Ņ>õƒE?Â÷±ß­òd?Àà»gÛš?ÞÛæ‰ü?ãñƒ²Éä?ר@†->?ÃK-^÷ û?Ý(.ó2'$?²øæý)ÕÊ?Ջ>bk]?±ã Û¾h?ʙ%Uzÿ?ª·†4O!'?Ãöù«˜?§o"¸v0?áßõÓ£¢ÿ?¸<ô'²¦x?ÒD—ƒ-¶5?²2;ò¶?ȇ8²½Æ¹?¾ã͎,˜?ã<I=Fî?Æ$U•ä{?ʇ¢X&?¿šÚ÷²Ô~?×tÕÕÙ?Í<¤¼ôxÉ?×[¤ÒvŸ?ÂW·X靊?Ñ0<W°Q?ÁºÑçW¬S?äñÄëyW§?± b/¦ßô?͘ýøÏñ?«üf×E¶?½Až¨C¢ä?¡>é ŸÅž?Ôi9!M?©#[Ï´ˆ³?ߊٱÑb¢?®Ð$Æãó"?Çëz*:!?¢)PK|MIXED3FGL J0818.0+3237@g²(¡ß¹9@?WG²JÀ:8CÔk&ÀÀ;çÖNUο©¢ñ^¶öu@!¹f"‡Ý@q]À¥w?ç:¡f—Ž§¿é©a¿Õ$¾í!g?¿èaFNm÷)UNASNone?ïûiß±o¾?:£Ã`Ý?"‡lX? ‡7Ztì—?;mx7]™³?5ý±q֟È?ïiÞCö-?'ø*AÉ®G?€Xì&ð‰ß?~åna?…eœM9Tò?¿†§Ä?ï4ï"Œ?"Ãq«}@?ƒ(ia]µ?tº²Ã?›Ò\md?|¶þ?•?î¶úÙX)?›×bUtK?x`>hJ^?sßÍf?ñþ?¡"JŸWëò?š&¶Öžæ=?ïþ))€=8?!ZÇþ?©Êqv;?;¶tN¼?#"îA£?V±©ñ•õ?ïɺhÉ?uŒP¾Ýî'?i(^;r8?avOß.­Ì?mÔç³åî"?q~µÇð–?ï›Uð¼/
?sB™OZó?u÷DÜǾ?fw䣐5ë?|]ӉÓ]?k­àVÏ?ï¿,jŸº?t̊áÉ?c7P³¨ŒÇ?Qà3˾?vÙÁSO8ô?r|vú«AGN3FGL J0823.3-4205c@p<†DR?hÀâøæ0K!À9‹j˜û)À:»Þzt¿ñŽ;AŸˆ@NûÆ_u[@~µÀ@ÍP¿èBS¿âÕ­›rü¿æ¹Lé×cm¿Ðõ›Ã?…QUNASNone ?í{'k:ò«?²^µ—üáh?~¢Ç3fyÿ?~ôÛÐ	F?²9À1‡,G?±Ö§"tÌ?èÍGÍZLŽ?Є>¸kø?–«88¼Æ+?žÀ§¶£ü°?ÉõyÃ5?Ï¥pxŸ4?ç(zxž?¶Ö7Kõ
©?³²:"±Gñ?¢½¬RÁ´d?Ê
A''?²´a¦±?ëùYÅeœ´?´mBk?98
þ'b?@)G‡VUÚ?À
üã
®?´‰VNz?ïËÙv˜'? u<¼9?jEHR׍?l¥ë}>?œÛÆÛ^E?ž¦áû}Ò?í/o›ÿŒ?ÂGô‹W·w?‰9³"'U?–¯tdçò?³c "‡¯Û?À'¼8Mç?ì‡)+6Sh?§ÔÑÐÄ?¡zò²·
M?"ù9`u•ì?³	=Lƒêš?¢x"ãÂÊ¥?îx_LÁ¤¦?˜6×ÓG,"?&yIX¯?…–œ´À?¨cクhÚ?˜-·'5ɧAGN3FGL J0823.6-4838@p"HýŸÓoÀ´]+TBÀ8ö$"]?vÀ:ó¸°¶Ñ?õAš	.Ï@þdRåÖ@æW_¸Lb¿à«l	¾o½¿ëÝüÓm®¿è8¢ÆœS¿íOÂNÞNUNASNone?ë_¯R
_?½ö'þUí?‡ó†<-?†2ô|œ¼A?ÁïoÂ?½|dzª´A?㽸;˜=?Ï£î@SÆë?¸OçÉeT½?³xþBHv}?Òp•˜œÞ6?ÉðÃ<™¨?çhCfs–?³›æL#æ?º·Qa,ÑÖ?¤až	"»?ÅK	Ïȼ?°x	u rÏ?â˶Mäm?µL5R"š?ÀÊçÙK>?®×!zý?ҏqw'‡?²Cb¯#xé?íøqèiz1?±2.çî©?íƒA6­Æ?=Ü+Ôâø?¬{1‹a·?°©œ½
Þ?ê—œÙ?Ãß<É?¬âžYí"3?¨mtú2I?ÀXùôÖ´¶?½»€3Áù_?êã–Y

?ªæ‹êŸ{?²:ï‰?C(Þ@s«?¶ÍU®z€?¤ 6Ž(ï…?è_çFJ½?¥¸¤éÝ=ƒ?¿\{V§? Æê jš?¼¨…ku€?žU×y®UAGN3FGL J0826.3-5056@pµìß&k¥À…ñ¾ôœõÀ9C¾b¦¾EÀ;*Aç+ä?ð¥YEÁ€=@a…'ͼ@ÓÖÀk•z¿æo0m
Ó¿È©ü¯#Õ®¿á¡Ôñα¿ïþCj–fUNASNone?ÍÜÌgTÖz?ÅQÞÛåf?æëÞU¾Öó?ÇKwþûYc?©Îéhä?©—¹G÷?ºB+|8=g?¼‡(¹CÈ?á9+/òa?Æ,Î÷쭊?Öýñ+&?đþFä¸H?ÛON
¾º?¶ÁÈ£!¢?ڇ2d ?µûÕC«á?Äá#HÊ?©TIwP?Ó·.;–?¶
2rIò³?ßh…EàÆ?¾Úõ0¸?Ë#‡cáüµ?³êÍ­;?ÔSp-B6?ÉÁ¡«o?åàÕî3¥?Êš%W±?š¬âj¦Ž‹?"+"rº•d?Ï@mØP'?ÅTâg`-à?Þdú¼½?Ã@Q|§ùâ?Ñûº×Â/?¿Ýö¢«ˆ|?ä­F7zsA?±¤æòXp±?ÐÝxÖ"?®§ã1;'?·íÚY?q?Ÿ|®dGvc?àVµ=†jµ?±øfîˆ?Ö¹!˜§=?²''	ú¬?Á2éµ²?£Ô˜¨jÞ>MIXED3FGL J0826.3-6400@qfþ=ÁÀ-L4"…ƒÀ9õVI¸±À;­i#L5¿÷'Ìg¢%¯@…×Sƒ¶@¼tÿ[j_¿èš¨
ܹ¿âs? (ÿÔ¿ê#2X(c¿Òpå;¿¯êUNASNone?îă1o±
?£°ºÖ&Ô?Û¥[-s?•(?dC÷Q?—Ç'âÁ-?œ>¤µg?ï
ñú´g?¦†n–!I?i…€a' ?'{ÕP»?–glŸVf? <c®\<?ìSc9˪?¥ÜóU_žo?¤Á¥£Ô`?'_îé\ny?³X…d±Å?¡ÕdpÏ?ºË~ª?šôƒ:«¤?QPB†(Ü?Z͟>Îä«?¤2?Eš?™ËϹ˚?ﯤïtRÉ?‰ñÿk˜oò?hµlnH?p|RmT|?|%-°7þ?…j3ãLå
?ï¾-¥T¸¿?"î½\.?aX9•^‰Á?oª˜æU?x=kWóÏ?}"Þ«†Õì?îӂ³ùí?ˆk¥¦©]Ã?Žâå'™?y@åœ~/Ä?–6üàH§?¦»Gi£?ïÂuüÛ?p pRkdT?
§ÖÌ?J o¿S?~PË-h(•?p	|>ã•9AGN3FGL J0829.8-5239@pіœ#·•ÀªB9`tÀ9rƔ¤gSÀ;:?wTW?×Ú+´RœI@
€ˆ!ö@}úÿåþÍ¿åöR­!¿ë½²8Ýþ4¿â5Ài;'¿èiÕ°ïUNASNone?åÖ(w‡9ß?Ð	ÄÕ1 6?…o7Jû}?ˆ"ì¾x®å?Ó¨5VŸ…?ÏïÊ#‹[¤?æf³V•I9?Îy<YL?²æ5XXYÿ?±àEy>¬Ï?Ìò÷æ_?ÈÞ—•ˆh?ê]¹\é¡*?«¬jÔ¬?¨pîD_¹ ?"Bj°8qª?ÀlÞûx†Ï?§—aªÈ?ä±"ÜÓ?°ò=ì^]?«–=ØHn?›;\ZE‡#?Ó*ý~ny?°	'¾-ù?ë4¡käÄT?я|ûíæ?z	P­Ý´?"(©'Êê?Â]/ÌÝyÿ?Ñ2]ç"Ê?ìuzµ ,Ó?¿-hKT"?Ÿä5I8P?¢ãA†Çª°?´[ÿÔ±Õ?·±{LLjÚ?îTd_"ÔÓ?"xígáŒ?'@ܗ"¼I?€á'^Q?¢K¹8†´?Ž­úÖsµG?ë6…^èÝh?œfßöÚ?¤éˆ<¡‡T?†¹ákH'?»×êÖD'?˜$úò`@nAGN3FGL J0830.5-4452@plÎp:ûÀ
Nb®•ªÀ9ò"Ýr6À:0‰ÁµA–¿ãö¸%^
@‰ÿÈ¢œ?ÿ9{ßto>¿éP¥:üD#?ï½jòŸd?Óa°¦Ûj¿èF¶]I²&UNASNone?É5©&¡Í?Æ:‹6mô?¢ÀM|Ø?¨YGÒi©?莭¼Þ?È+Qÿôcâ?èÉwŸ7­?ÏâÀ‡¢©Á?£«/鶴?«VN6¼!?ÇïU‰…‹?Ì*€b¢Ü?ÖҖß?²¿[°Îì?¾#ŒüAp?ª_i?á:ÿ÷,Øâ?´û½æü:?è1ŽC?Ì6"ž~Þ?]{X€g¡?""§¶> 7?Î#üóAg?Ì$üí.Ÿ®?ÆúҐþb?Æs±Aoз?œkŁòŠ?¦&¹EdÝ?éšc"ô»?È ÓàžÖ?íÑƺA¸?×ØV÷;>?"Pò2xRk?¤ž}$¶D?²55=ýÑ!?À
㚳d?؛›v¬?´©e©÷S?¿«"~ãú?¨ø|:ÿ~}?ßyµãý?´Àº¤¦ôé?é£+R-
C? ÅMãžÝ?y`*©I*?{q*Ó3?Ȫ¯¶¼j)?€@JPŽÁMIXED3FGL J0830.8+2629@h­>À//˜@@F¾œˆacÀ:-Ü^:GúÀ;Ê zÉʺ¿ÒŽAX²@&@HNx^@tPÿ÷Çw¿ækš
+í¿é*l{¥¿ÜrWÙcg¿ïÿᘴ(UNASNone?ïÈû¤'z?"VŽj?JDE'xît?Mwn†É"?x9ôUaG?ƒØ#eˆa?ïTu*×ù?˜hغÿñ?ŽOÓXÖPœ?ˆ²âÀÔñß?ŽÛNµAV?'²¬ç´?íãOüÒ?š÷W
M³w?œo#ÄîA?ˆfܨÃö=?£Èօù¢Å?•VŸ–±?îK¥&âå4?™Í+q'Ël?‹``¶û´?†¾þððÊ?¤m•c6؛?"ýâ֞A?ïïV5R'?gŽ'BP8?6[ ERGè?6Öl¨&÷Ê?[¼­e–lD?f'Ô³,‡?ï´A7z7 ?xïs/†?r¶¥;3íÎ?fRÞÆʦ?s(¿'Léö?sÏPe>?îÏûäE?hÔC¨e(?'öÀ(^í?|`o'C=ß?"	ÃIה›?ˆ	'–ºðk?ïŸè?ì?tŠþ¾ô?pp|ˆÊf?`ûCŽÙÐ?€¹—AÏ?pjÅD

>AGN3FGL J0832.8-4321@p]1¤½º
ÀzMÙ§¦£À8ßÕùµcÀ:p•âTô?çžR@i§Ž@¾½Òß@`•ì翌»Ë'%Þ¿êFÑËå¿éô{Kû¬¿ØBR'X"¦UNASNone?ÐÄF%†Ö?ÅlŒØHµ?¿®ª€zA?¾$ëdðù?ãº^-M?ÊêËOõ
Ù?ÔÃÚhtf?іIš !@?·˜
2Qïˆ?µ$šˆc'?ãÌá¼ë?Ðîý(»O?ÕXÓ4‰¹A?¹1ãÛÒ¼5?ÂàÚÁ<–?­8c1žJ¾?à›_µzÔ:?»0ï®p©?Ôj£\ð$?Á{b&?¢FLf§¥?¢æ²Z"p÷?ä¦I®}_?Á€fNµçû?Þˏ(/&½?ËþÓ¸¬âÕ?±Qƒ•š?°êX¹Â"j?Üà)vý?ËÈ¡NÄ´%?áöA¼Í?Ó¯»	xF?±ÝïL
&?®ŸÈL~k'?×°}?ÑЌ·€VÊ?ä	aJC?¸hŠM?¹P¿ÑŠÎ?£d:éÀ5€?Ñ·҇ˆ?¶eeÞ3Û?ßן¹æ…?¾DîÜít?£†ìï‡*å?–çñøG¨?Ý·ƒUp°þ?¾pßóèfÿMIXED3FGL J0834.5-4825@p¡JB®Ñ9ÀV¿2/'À9hhó ¸À:Äþí±Hã¿Âï÷<j
@Áe¥÷ @€w´—¿çŸÊR@Œ¿ê¤€HBl•¿ÞŠz܃èÇ¿êl¹oUUNASNone?ë0ÀÚ¸ë?¼Òï)V?"»eY;©¦?•·»/ÐÚ?À¥ë‰À"?»ë;§æç?êLÃÈʽ1?Å;Ę1ï?œåFh‡7? K`n³D™?Ã0MÔãáU?ÂÞœ2#?ãїŽôÇ_?¹>ç:oA?·•ê^>_ó?¡½R@Òt?ÒwVJ†ÙE?¶{®WXæÓ?åÌ.]Ð.›?¿uºF¿?}D=i¾oÈ?sè#þ+*?Óò'Nv°‹?¿0»§¾þá?í¤·µ8†"?µ	ÀÖÆâ?ˆñîMŶ?"š­M¨â?¯x	ÍN?²ð¹J•Îª?î-Š¹p¾H?±uý25Ö?†­ˆ² «?‹ïU™×°?§{òd—÷\?­«¹ž'Œ?ë
úãò"n?«÷¯òž?¨ÿ¨™Ì S?—½)ÃR7¡?»(Tƒ£í?§ÇvÚN?êëãš]}£?ªÓÕøÃ?~F¦•?hr­ÿé?Ã^<`Ù^¬?ª%™ð$ºAGN3FGL J0834.6+6101@cpŠGìþ›@AõÑN;Í6À:'dgˆ¥VÀ<
n.±Ä3?Ғf)T¸@Ëg!wI
@S;ÝÛ¾¿ÝpÑF⛿äpÓàx"¿ê'ÃC-ž–¿ãM®23ËUNASNone?ï¬÷šU×"?'áŤYÒ?}Iy¥™;U?aÑÆL¦/?hurŠñg	?cæÜÐ}?î)Á£*£?³ï‹+;? Ø™­½G\?¬kIÂDGS?™©P ä?¥˜q)Ò¦?í0­h>¾é? A?¢N5§ˆ˜á?'&'û¼\?ª¦óÐ?õ™?"'çPû~?êqÈv?¼?³
G^ò¨?»¤Bržá‹?±~=´]Ô?°ÍyØψ–?¢èFöÂ?ïé¶UD³—?dîŒ_©CÀ?Z*ç~æ¥:?aó´ÑÜ?Rhmy@Ù?N}M?ï‰lBüÝi?•Ò]pΓ.?€&Ö]a0z?ÿö?zü1¹zr?†?ól!ö?îÙ5õ@š‹?ŒëÌ­v?'ŠØ©
¦?"ÖƸl?"N±†"Øî?€´'º±"Â?îܹQV?ÆÂ&-õ?˜VçˆÞã?…\ñ›P?ˆM'Œ.C'?€µW	,¸AGN3FGL J0838.8-2829@oS\gßã*@4~êÁªÀ9©Û0=À;r-͘¤§?òMÂÎq<®@â†óNÂ@ÌÞࠔ5¿àth‡©¿àƒ÷à"¿äŒÌV°;¿îG\sQUNASNone?¤d{&RTU?¢*ü·2¤?ìÐi§ŽyÖ?³"ÃþÚ×v?®"ê^2YQ?¬Tàgjd¦?ª\: ?°5Fr
@?åM%·
ŒŸ?Æ÷_#Z½?Ò%1ÝâŽ?ÆióZˆÀ?ÓÚ¯^&üÄ?²«r¸\?ác|®ž°Ò?´Ö1øG?¼®‹]­?£)fl×Ä?Ì%§d2"?­/á2ú"?äY{½$Ó?´gj$§xV?Âtl>þ©¥?©"ûÜ<¨é?²L¹ˆ²?®à±¬Ç?ìOxÈ,˜Ô?´¾ñA÷?¦ooºÃ£?¡ì5.;ü?Àxóàüže?ºèxË!?äLXe™¯?ÖšFMþ?ÎU«ÁlúÞ?Á>äy3??â1¬d;X?³Ï	;]¼?ÕÚï'âÑz?±<‡EÞ?·â´'œ¹Ú?›.Ý|§?ÝÏ<[Ùx4?¬®,Ž7î?ÜóõÅz¯?¯7Ah]À?´ö–»<o?›œ¸üÄîMIXED3FGL J0838.9-4056c@pI*â—9m?Ó@¦¹<ÍÀ8Ð/9©núÀ:mSB3'?Ä\G‹|Aç@Ù@ºZYh@MüŸù/+¿ç×{ÉÇV¿é' ÚE¿ë³3§*¿æâÓUÁÂFUNASNone(?â¿dlĬö?̱¯Ì4?±V£l)"'?±ªÚrr{W?Ö+ŽJþMp?ËÉ–£3æ?ÀԎ'dHÕ?Å/àž?¶Itt8dŠ?²Ÿ\רe=?é­ÑMÔ¹?ÇÌ¡væCõ?Öá¢^S?¹>>±
g?ÆÖò³;?°ïMãÁ?ݳâZ¨˜?º<M¬8á&?Ø"ܽÓ?Âl•ˆ×™? Ñ÷!<Ä4?•ˆ'Àtj?âñÒl?'ñ<ÿËä?éÞÜ›?Æé³ çþ?›Ú'®·»?¡*J†ï ?Å	MÞ§?ŋw¯†bR?ϕª{§…?ÑÆ*\Ü
>?·ùŸx1¾?ª5sõ;"?å8V'ÿÎW?Ñö±v?äpÂúˆ?¶Úܯޜ?½¸ê¬Ž?¦ÏmÚŀ?Ïa†ž—?³/U:~‡ï?á‹cžé?½Î‹{ï¡?˜ÈYå=uÆ?ƒ¨R"[=Ä?Û\´<nV†?½N
²£´XMIXED3FGL J0843.4+6713@by•$Ý@A͂¡ ÏÀ9¦sŠ;WÅÀ;Βßk5?çÌ'æs@uÞ©n#?ÿàß=Ù¿æÑ´¬ß5¿Ü¬È$òRÿҜz¿;Ù¿ìº9$
üBUNASNone?í#rXë‡+?´{G»Á¼Â?¶¬â0=?´"궠C?jª'³LS?o~àŸ)]í?ç™ÈÀ›¥?Çh'é!?É+@³×æå?Ä;62¨/?°Û8"
?®é·á{?è✇,&?¯µ4T‡?ÆIëÀq¹p?¬V¯–'¯?¨®ˆ'z	ˆ?˜:hº1GS?ê̙üjõ?³)_^å?ºȒ'£½?±úÇÔ6ñ?¯*ÏTÑ? ‡"uôbŽ?îFÖZ·}ý?¨ú‹ýÈÄà?ªZÞá¶ä?¨T낯;?c{·y½?cë§ûQ…‡?ìšHÿUéŸ?¸X<‹"T¤?³ç·þ—FÄ?´!܊	L¾?UM?œ©×Dîô?éñÙ¥çõa?¬Oq`Λ?ƨrœÌ÷?©yÆ´g¢½?¢ÇÃ×é]?"-yI'Ò?îÔ]²/4?–0xA$ûr?¨ÝíMÏ*p?'øqÚý€ä?ŒS3XÇí??€\b!¢WÿAGN3FGL J0844.3-4741@p§Î_oÒÀ¯ŠúšeqÀ9
£oÜ0îÀ:œÖÒ	L°?ì%p|ê·@H©}è88@±>ÿo6o?ïÿ¡"uÿr¿æ%ºÃϑè¿çŸd}G¿ìZíß
Ž€UNASNone?Ü9bã¶.Œ?ÓF×£H!µ?Þ¥w¾ê?ÒÑiR»?´†R•Ô1(?»T1°|4.?ÌDßá…@?ÎÚ¯vÙ-â?ÎOwÅh?Áq˔"uh?áZà©M–·?ÌÑLº÷@?ўÝ5z¶*?³ôÔµ2ö?ÕBeìª?´¹ôTÿuf?Ù¼ÝÛ+Ï?µ"Ú¹Ìd?Ãÿ܈pk<?±LûONï?ÏÍ
wÀ^ˆ?»>"äŁ?ãÅó͏?¿Ûûœv¡?ސ:¶±¿?ÒÚ¦˜õI?Ûü
'm??ÒS®þ° ?µÎíaJ{W?»'¨µE?Û6Œ¨‰:k?ӓû¸¦,Ù?ȣ̇qg»?ÀFÇuŽ¼?Øw«0ù?Íîq鍈û?àK.ÙvM?´™x«9Ñ?ЂÌü¦ö?°¹­?¦¤"?Íͪ ÛŠÞ?¯ýp@ RG?ÒtPÊGâB?´¾5úˆ¨Î?Ê1Lj\?°²ÊnØã¢?à9""‡È?·¿AqTûMIXED3FGL J0846.8-2638@oFÅCk›@$ªkøvžÃÀ:–ç7²À;œ}>ïÿØ?˜ÌÖõÕ@Ð3f´¿æ@ÈX *,y¿Ý´…XDοëX
Ò?l@¿ïÿ™]-š?ïü…û4Ç»UNASNone?ï
P¢$f?¨ÅzaËÉ?qKLÀ\*ë?w|°N?šc'úŒ?§²zÉv@?î13"[
‡?»-ƒ›‰?'—EUP?—_ùƒÇÇÁ?¨Fü¯èÇ?¸VTMô¥?뇁rË|?¥ÃÂm\×?¤©<óÓV?'³XjKäŠ?¹oUîtu?£øŸZñ
?ï9*S:º'?žá'¼Kd?Q*=Áæ?p¹I՞ô?—ÈÆßä?ž…³¹€j?ïÍ<埽±?‡bêÏÏÞ?JgEó);?VQÎÐW?v¤«‡4?…ÙNPË›?ï" k̊?¡ì˜iÐÆ?jVÛàzC?ƒù輧?"¢FiÛ`Å?›ò 3ö(p?îJÇ[ôv?'™žs´\Ý?'¢õºŒh?WQЌ™?¢cpç?0FbȞ«?ïìHÂû4?nþò759?ì-s¼?:'ÞPçd?bè°™ä6?m½¯;U
ZAGN3FGL J0847.2-6936@qÆð:û~'À0@ ÇÀ:Å~#òNÀ;¹ë˕•(¿õ¾"_¦XÅ@™ýAµ@4÷ 2z|¿êu)6Òqt¿äëE
¡¿¿ë	õûÖ`Û?±zG(ÒiìUNASNone	?ïð­H'Øõ?X¢»`:?K{ºÄDÎ-?JMs~?P瑘ôü?PŠ"4˜?ïxãÔPNÍ?Žµ1r
V?pT7ì?yk9»ْ?‰½J7'"?ŠÌò燛è?î`A}g£—?¤Dÿt¦?"I‰û…·?€îÖ_ƒl?Ÿñ†Éh?ˆ$<Ë7vd?ïµnqw¼z?~<[˜‡–Ò?™s§Â$F?#™JŽ™®†?'{0ÂÔr&?~,ú/?ïù"0b¸ ?Cí•æ›?3‡eD¦?1ip÷J??ߐÀÞ?<åJ¶©?ïÓßnÌ!½?sl
?VÉZ€ïɐ?W#g1i8ç?p]òæ?o›†h@Y'?ï[OzTC?z;æë–?'ÈvÆÕ°?r6‰Ä¯Zî?†cªµ¥Ý­?mváqÁ+¸?ïõ"DëÂ[?NûÚg"¦>âÏÛQÒ¡>䚽éގ?T³Ö_1c±?N㝗'±AGN3FGL J0848.2-4524@p'3]$žE¿ò.Ñõ*¹èÀ8Z¥öŸ..À:AJFu/W?Ü[wµn6i@*°ÁÔKF@:3q¿ãΞÜØ¿è‡Î¥%O¿çÚ¸'›¿æðu̓tšUNASNone?©Ùûù$‹?¥ˆUåh9?®µB"™^?±´äLV?ì€tì)ù?¶†'Ó?Áë0Sô ?ÃáIÈF?¾\ifº¸è?¶yϱ8Ã?繦¾+…{?ǃ°Î|?È¿v
ž?°?!‹½yM?Ê!€ˆ?n?µ])´oä?ãGÛÛH¢?¹çžMk»?ÒÚ#ޒ®)?½Ùˆ(ûCO?¢€žé<h?'¾®2¾—?åjä!Ó…?¾EWe˜?¸P'©+?µTøL¼Íú?£cۖ›
Ô?¦±Ò!TÌQ?ë¿Át\¦Ó?¹l*j?ÐÙF"Æ?ÎT{¦iŒ?½Œu&¦;?¯ÅÑgނú?ãáÞÐ8Õ?ÍÿÚÝ
?ÔD­[é?µ$]˜<?DZÛÚ±¼Ñ?°Ú»8Âí?àæ²Éb×?¶ŸW¾ØÃP?ۍ"Õ^¹?¼¦H®¼ä?£šcøZÁ®?ˆƒ'©âÓO?àÿ—UOEk?¼
^jøOTHER3FGL J0848.5+7018@brGE8ï@A•"Ý—ö+À:€€VÒt¬À<i[
lÐÀ‰©6šœ@ýïÀí›y@eÀy,g?ÏM¤È½|¿å[¦‡ÙL¿Ö0«±LO¿ãl¥‹«UNASNone?ïüô«@¾•?.6â=Øë?œýàS؟?m̲] ?2sf̂eF?)ÕÐDd(?ï¸'E-?ƒãO¬Kß
?m›yÄ¯D?wŽöëÀÁ?u ¦ìyú?zÿ=3Nxi?ïhÅoô?{lfyá?{ö·Ñ¢?k­Øëg
\?‡ÿC5—Ž?t.þQžh?ïá)T{ò?mEkŸTD?ë‹\d'?
ð¨YbŸ?n–[© ƒ¯?m)0q«³?ïþ7? @+??—U?O€@a)ö?	ÅÊ'Ôë?"äP…4?¼''è`?ïåkú?fw(§PRß?VtUwÁ?Ssà¾ú°?^¨zﻩ?`w[¶{?ï©ò³ú+?m­ïwŸ?r'!…¬ÁÛ?cèßUz*Ê?xt"Ôi
?cBÏFpp	?ïû}ïïç"?A£AQ¾å­>ÑTÃ%nZ>ÝI4¹K°Ä?Aå—k˜9…?AšÈ4=ÒWAGN3FGL J0854.4-4404@pŒîËûµ?âRuÚÀ8"­¨DWHÀ:DUFƒr?êOI£Ú\¥@¤'šG@Íù ?{¿âªÙ-5ö»¿ê"¶Êh*¿ëÅýÅ_'"¿×1¼áUNASNone?›ÆÄ"˜×?¡ "EØãm?­Íæ¶?µ—2.åìe?íDøð—,W?¹G÷fƌ?¼O.4?ÄQÔH—"?²ÔÅU?¯!ü[: ?ê":]Q_?Æx+:o+?È"dÞâ?®ü½#Ž.ê?ˊùÇñ_˜?µëÀ‹î?ã¨V~oz?¹®îCÙ¸\?×R‰º©^´?Ã/ªÔÄ,? mE"—Êz?¡þ‡ir2Ã?ãOæÊFW?Ã]q;<Ó+?¢ì«_JÛt?¨7Fãö&f?¥³^~	?±zæTwx?íuüt7èØ?·WËÀs¨7?ÌCsßÃ?ÒV$"¡ø?´Žø'šÉO?¦~ŠY좮?æ]CõÎ"ã?Ñ]vÑv2j?ÓSîŽ,lß?´'¨Ê}Öß?Ée~p.¢f?²NÈ}]
?ßùR9¼Aî?¶ç<–õ'?áK#™¯‹k?¿Â$}7ä?¡ÈRR}éI?–#½DO­k?Û0®'£¢¡?¿ÎÜJÝãMIXED3FGL J0855.4+7142@aÄû~ÿ—@Aœà\̉±À9²õÚPÀ;¾½Žkh.?Ê*êdbU5@_ÝË¢«;@"5`4>¿âÙ±8¿æËÜ2¬‹Ë¿æÆCG¿ïÿêaïD'UNASNone?ïžLlP?—ªv¯¶pÓ?Tˆ˜è1?dÂ_­,ýô?…èË
Hæö?–øEÝ
?ž"¦"?¢ô?.H{?™Â_.»^£?•xNrC?•¦­ÈfÛ?˜û5YÂØÇ?íâǾùƒ?¢¶3—×ٍ?˜ÄÁÐ`ý?'2­'¨q?¥u¢ŸuÓK? ï>kêm?ìÿ£tll?£ë#±ØL)?¨|7ÏsFÿ?šƒ›§ýÓ?§‰è)‹?š ŽëD?ï¼GÖ¥¶?'àgµü
É?WÜié£Ö2?t‰4–"'?{úÁ…¦‡'?'f<"q"?zu?…i7öK?€ƒw+ûx?yÔvŽ£ƒ•?|9ÍB­=?}.%ƒýc?S·"‰?˜¡ö'?£œ?'è»
9'?Šûðª6E?˜aZw•™Í?"©M{9Ûd?ï\Îg™s?€éŽü??…Íëâ¾[?s$ô™)
?'ÿK$ð"?y©L@՛AGN3FGL J0856.4+6429@bÔ_Eà´á@BÏ …±…IÀ:wÖ²ÿœ-À;þ¿:=°¿£	ëû·@±¯ØuLˆ@iƒÿÔa¿ê_]Zùö§¿áÎÂ7óaa¿ã=ÞNn;â¿âˀR[þ•UNASNone?ïùRºÀŽ?E–Yà±7?72"½ÜÀ"?8¿¿^8üÒ?@rØ%¾?<º="¨©è?ï{•l8–?']4P?}Vo¨Ð]l?':nΏ?'o†Kº7Ò?‰lr·0?îÇÅ&^B?‹öG""&P?FEȦw?{œvÓyïÅ?˜d8´ˆz'?ƒ4×Î_«V?ï:wÁhÑ·?‹€|¦¿}÷?{Ž~i"¬a?sëKeøŽ?'Íh9`…?‡4W$Èð?ïüÁß³Ú8?2{2¡"ˆ?#¸49è¯?'ók•ó?0d¥ÅSBÄ?+	4^çÎÿ?ïÕC—)7?r—d4+Üu?cMÈ~Â$i?a}F–Ù?gn œð§?j"‡u8ì?ï´°÷.J?uP#>؇³?{%Œ+œæÖ?iM5"æÌZ?'€
¦Ž¤
?lìˆ?YP6?ïØÐ`L"N?fE¨}ýyÅ?aŸ "+š?MÃ!x¹?fDÄæ/?b&ÜU[AGN3FGL J0858.0-4834@pÊÅXd¿þc@A8¯À8÷0t<ÿÀ:T¹¼NÐH?ðjÓ*‰ìR@
âjé,)@•ô@")›¿é¬p®i¿Þå;j܏/¿ízíBIb¿æ#}"ÔÕIUNASNone?¨Q|qÂD?¯m!+ùÌî?âΝG§h?ÒôR~8Pe?×X¢aH?Òhãï°?ÇØOË"l?̼G•&(š?ÈJÀªYÁ?ÁCŠP6µ?ã÷<è5?ÍÚr¸ëT³?Ìr'ëú†ç?±Û,¼ð|?Ó±JsIVi?·w›¸,פ?Þt¹f$?·t'qËØ?ÄèÆa?¹Àxx>E?ʑÝ)2Ì?¾9#"é?ä*øž"1u?«rES–?®µ'ÏÞÂF?·S#ûqv?á@
ï>´?Әý6ö1?Ù©E(~#q?Ò;Òh'?×hôn?ÒwüÏ&¡Þ?Ão×B5sn?¼¼»j1?ÞàÎUQÛ?ÐXðA?ةѵ"ÌÖ?¹gӝÓ8l?ÎÖíÓé²È?´ê}ªkG#?×ê·`vYÆ?¶µÏ҈?Î*5.q=Á?»[ÿ£?Ê)Wý—ðÍ?±"žƒ¾Yû?áë´ý´\?¾ÎåráMIXED3FGL J0859.3-4732@pÀ
»Då¿ð¸±§­X"À8±öFBÚpÀ:J­wœï?ëñ&D§Ã@
2L["e†@^¡`^x?š¢öÛ+C׿ërò·~B6¿ârKuãö¤¿êM|œÖUNASNone?'~s4jiÐ?Œ´	åå€+?Ç»\ƒd›?ÇãNÌõDC?éÇ/2-àÊ?È¿^q? ¿‹9µÑ?¬×b¦3?Ë ɖ¿þ?¾WH·åñ?è,\v´£?Á¢_µa(?ÃD…Å@*V?¦©â£4V?Ð~˜Nã4?±k[³Nk?âïÑÃô/?³
ÜOg??¹éTŠúM?°"8RñƒT?ºD™+"?©õxE>¬?ézBL'å+?¸hE­—?{E8vòƒH?€"4æì¨?Áa~±G"?ƧÀ–çV?ëqã'h`?ÇvËÕ<C8?²Ä–ŠÕ+?ºL<¯êÛ?Ípóחoâ?¹—©¦îF
?æK0Fˆ"R?ÄqtjÌ?Ï×À¦xÐ ?°º	tµ?Ë딻/ãÀ?¯jOä+??á*§•Ó?³±¦ë¤™Ì?Ã)ºT‹XÊ?¶ ܬÇQk?ÃÏ­/+?¤¹'¢e…?ænÝ'Iƒ?ºJd/ÝñÁOTHER3FGL J0900.0+6754@bL"‰a=@Buk¹Œ~(À:ùÂÏ	À<´æüù»?Чɧ‡@©(ÃBµ\@è¶à|W¿Û|õĒÁŽ¿ä7æN†©[¿ÜÉnûØ b¿ïÿ™äOUNASNone?ï‡6‡åü?Ãh#0Ý?ÿXy˜?'&YH(?xe½¡0®?"ôŒèS?ì<P<GG×?µa¶L"r?³ç>Ï.âþ?¯xk"ªÂ?¤l~-¼–?¤
¼]í/¿?ëٗñá?¥é—¨ì?µ¥æ‡à"ç?¡$/3o$B?§Á Çr?"³CR©ßÒ?졅c¯˜?§ô¹æO˜?°N™!®äJ?£=ô0ÖÇ?¥Jw‡öÙç?–»öJD&?ï؀Îá=â?k𔭗—}?eÚ¿ý")q?d5SÏ­ù?a¤q+>ܯ?Z8	wž*L?îõصÊbö?–#Ä›(?"¾×
9ñ¶?Ž´ç'ìÙ?‰$vbúú?‡2´$¾?íçµ…Ðå?–xÿßãn¿?¦™ÐÁ"?'Ä:Ö5n[?•Õ¿JêE??ƒüU³á"€?ï}çó€?"rÁ—´$?•jL˹?ogEÑ?€'}álíð?uù° <ãAGN3FGL J0901.0-6725@q·}'ÔÀ+ˆ}€^_1À:D!BoçÀ;ºÉ«¿ñ0Ìxéö©@
AK<>u@0ـ9vC¿æS÷'.|{¿åƒéY€ú¿è-h+•¿äGïç?PUNASNone?ïžH[t¬?‰!´øÉ«?Zi7''Åâ?Y¼Lº‡?… Â9Ã<£?‡~Cuø4?î㤍²?¨j
'¬ï?`"§b@¥?Îûöçñ?šÛj¹ 6p?£U'Æ4۔?í#üŠÎU?œ×‡zƒ	ý??-ß®ž0?†ìq,èì=?¯  i¯€"?—…傇L?î‡Ý{_‹›?"'î†?e¤õƒRlù?c¶ÜIé?a?¦'Øó1÷…?"ˆZ6–?ïåÅè4ºÐ?ha-·´:?C	X]ê?CŒ¦ó¶í=?eYÕ՞š?e±ß†Æ׸?ﰃªçA:?†Ýói-eö?d¡7ûËd+?ndÈE§?}mŽpí
??ÄYÖöõR?ï…žK@?"ób?ˆÆ'ðpý?ríSœ‰Š?'¹Æƒß'€?w(ÏÚVÎÈ?ï´~Q¿N?ouKYû=??¾Šœ·l?3ùœ+¡ÆÈ?âw-Yç"?nÓë¾NGAGN3FGL J0903.0-4826@pÑXDЩ¿òÛç‡c60À8ÓÝËø'wÀ:Y8Ëùh6?õ(Ve½I!@
3´k×êb@¼2@·?ê?sÃq.k¿êIˆÆÒP´¿èLd¤LD¿ïÿæ
æÀUNASNone?k¶JlÒ;?ƒÐ'EÍø?µ—DC•šË?¾ò|V47?í1aanÚÔ?¾Òå;iÉ®?ma7ˆƒÐ?‹Q@"'g?Þ9x­Ìè?Ä9'F…:?àÅâø¶?Äa‰"<2?·8s'k´?¡{1¯½Ý?ӄ`Áz¢ø?³â©ÿìˆ?ãVÁ:Gy'?µ<./Ûh[? &s%Ib5?":4ÇAyp?ی´&kWE?Á|­÷/Ýú?á7>º>Ä{?ÁÃQm??kŒYõQÁ¸?€'huY½?ºÂð.Àw?Á•\ï«ZH?ìŒ3ˆ S?ž9—Ó?~ØÓÛÿ®˜?"¤±Ö³?àx‡‰)g‹?¿Æ†Ïšn?ޓÚ=p?Àk3ë{Â?Èö/ ñ@Ž?«³yEvî?Ó´ÎÝâã~?°óíd¿>¼?ßÐQ¤|:?´€}Ì"à?ªZ4F1&?žöˆ½¬¼?Üo*¦'òI?¸1Ö½ @?à u	'­)?¹ɹž§MIXED3FGL J0903.2-4744@pÉAÝ!ê¿åߑ€EŠ¤À8­XIm1\À:\ƒ‹:[F?óšzí±ô¯@Å·n–¶@Aäpb¿ìˆÎñÅ+?Ð$fJÑyI¿éKÉ®¤Ÿ¿ç;ý8>N´UNASNone?ÙÌ_ú'?ȈÆ¿+?ÔuaÓ¦ýþ?É*œ.Šò?Ѿ>1ǀæ?ş6ë¾Ca?ºË:»è£î?ÃÎID"^?ÈØÖè¦ê?½ŒzØ@ý?æ ârÈÁÈ?ÈÆ[T˚"?ԋ¸~ûÍZ?µœµdZ°k?Ñ#ÛÐ("?µÑ¨œ\e³?ÚPk°Û³"?·º÷§rÉl?Ò~PDˆh?ÀÔ¿Ä.?ÖRíHÿ^?ÂE%$k‰?×.ôf¼?íÎOôy?åDð`?ÊˋáÐ?É0£$́è?Äúr›í œ?ÂjI·L™?À<PÍ;ÌN?Ž³Ì˜?ÇD#‰r?Ç݆<‰b?µË¸¤Ç&?äÂïêz?ÈÉËxíZ??àÐ	~j$r?¹çH¨T6R?ÆÃ:Ôߍ;?®žr'ý…?ÒþO™ÎÑ<?´ÐŒVo`Q?څÐDÚ?¼¥jŒ™'?Ðù7ûU1œ?³‰'q9Ý?ԁ·òíjI?ºÛÝmÑ65MIXED3FGL J0905.8-2127@o'>E@0òædM‡rÀ9›†g­ÓÀ;}´{/P?ó6Qbô@xè±Ú®@G—¸òпàÍ,×Wû¿ê~²Ó¿éù{ßýߝ¿ïÿJX=ÙªUNASNone?èÄ+SžkC?Á¥[¨·­?ÃDÄúŠ9?¾Š;œ}?³Up‹è³?®+ã˜ø&E?ÓYc¹bâ£?Ǘ™àÍpó?á¤ÐVų?Ç«2øi¢u?¹÷2&í?ÀH†i\?å{z…éJ?²ðgñ"Ç?ÌÑ|"Õð?¯Q+©—?½'+æ&©Ò?¢/ñXt?Ê°Å/Iš?°
#ÌZY?仝u¤Ðb?¹䥔K<?ÂòÙd=tÞ?­Õâ†Y?ìuº;re?´Qó;Cž?´:DüC?±2ûW<>? /YÄHm"?š}	c5è?âŠðÖ0<£?Æ6- þ?Ԁša7ó?"€²ý³?¹¦ÅV(?·­(ô×2?éã:à¯?©¶[d¬\?ÁJÛï20?¤'lj1X/?®¤&øÐî?–—²õÇS!?Ý4¾'mò?­"Ú\¨?ݼMùˆº?°
‰§mƒ?´;Ï}WùÏ?™Àá&ãþôMIXED3FGL J0918.2-4859@pó¿3‡?҉O_
ׄÀ9.‡¶BFÌÀ:¥£Ho?å¿ÖQ¶@
ÀÍ^m»@†Î¿Á œ¿Ù Ö²÷¿æÒáìĎæ¿ç¶hK2¿èýI¯vz±UNASNone?ÓäÎщÊï?Æ¡( tý?ÊyIdob±?ÂÞlÕ|…?Þތ|>ƒ¸?ÉYiLcŸ¦?¤é1R$¾?±"Eæ^ü?¿•³'›˜?´4M7áÜ?꾸·ìëÑ?¾ðaäw?݆í'"ËW?·¨4´_'?ÇkÔ¸"?±0ïÂ2NŽ?Öð\î\X_?µ
šˆD6?Ó¿x6¯?¹Ød|[µ?¼uòS!è?¦ãÈrè-e?âå=Õ߬4?ºáa'6ëò?ãsÁe»p¯?É¿ö-Kñ#?Á%+¢^ÿ?½î½ãOñ?Вjž·ï#?ÄÁÝ°¥¿?½Õy(

?Æ·$¥Ñ¶?ÁP/"õ?)?¯"ÞÛÍX©?çñPϝ®ô?ÉÐ ½€®?çˆÊ¤~z?°‡¯}¯ÎÒ?ºGÄBm@~?¤}ê^)Â?ĸóNõ90?©4tp‡?Ý´<ØM‰?·m/2'…v?¾ÄÃ¥r?Ÿ~y3›Ù}?ښ¸ÙáïZ?µTX7r´³MIXED3FGL J0919.4+6604@bvwFˆ{@C¬ü'œýÒÀ:§¢m}±ÝÀ<»%}¿ËDzfoÈ@Øi2ɀè@DÀ
¡©¿ÞºÎ}Q¿×:´Z¿Þï`qH±¿ê÷Ø'D,UNASNone?îçK'"[†?£†O8B(Ô?'6Ìu[?''Œp?ßÁ8rvæ?ŸïβêžP?ï¡×oÝ?£JÿCÒ|?'ëO–W?@ÔT­5Á?…‡?¯*k?#Ž£¼ö%?ìK¸E?§[T€e	?±ë%íï??¡^óXçG®?ª•d'ä"?›ûp&Ã3'?îÃ:¿HÅ?'Œ¦é©Ë?¢ÊO+ý®?ƒh‹>íè…?–õòóÃÉ?Š2èÒÀ@r?ï}Ì&½6µ?™nA4[=?ïü3?"£F-Æ=»?ìÀÀó?•Î}"˜´?ï½¹É\LT?w <8P
¨?p.ԙìÅü?gÀ%Q»³?pôF¦V?qZÅQc	?íéè½c?ŒâV?àg?¤a³K0Ø?–Ü'NF¶¨?™ÿ'<ì֔?R²–†?ï¾A
P)Ó?m,{Ù¾?p
@ŖòP?['*+Tœ?pÒ:ÔC?fLlý¼ÌAGN3FGL J0919.5-2200@ol¯öÓ0"@3áÞ¬É!À:qÀY÷ÃÀ;¾UË
¯ì¿Ô9Þpì¯Ê@ÿä8¼µ@"ÔÒXR¿ïûM˜†–?ïMÁ`KÞ꿬ŒáõÆ6¿ïÿÚeÌUNASNone?ìñX=¿åD?½Ü	£Z?¦+]6HÒ?®¦.ם¥?ª¿ò+é?·:/YÕvy?âSçü±Ÿ}?՟µ]ֆ?Õæ€@ñу?Ó؁ Bnÿ?µÆ¿	
?µºÉØ
Iƒ?ææ·;ûÒ?³þaaÁQ?ÇéL¡æ''?²ªðîýê ?¸÷¬âÉ#Ð?¦qtðïv-?êíZ<a…?Å3Çob/í?À}–n@ûH?Å!º§}ªG?žraMK-?¡¸ë|6óŒ?ízFf'š?¿oBgñ?¡‹»ŽÐ¬š?®vp¿m¯)?¦ÏÞ*ÔÂ?º½¼Roþ/?æï¼2m1ÿ?Óß"Ìç?Í42ý?д]?KDw?¬Ÿlt÷?¯e&ô?éÒÜïI³?¬RûÒf?Á·ÜZ‰cl?©Iށ'KS?«ò¿œ)ð(?›	ƒ/¡—?î觗Å?K?¡'j™uJ?™ä®EB^? 7Ò*3ú?'½•Y¾l?J¦R ÇòAGN3FGL J0921.6+2339@iœ´¢3œ@Ej˜þi'À9ØüvÀ;°jš¸¿ãðrô
Ë­@FŠ{ïd§?ÿ¢Z± I¿ÐÔò׿´¿áéÈ]ÒC.¿Ø¨b†¿ä<+{.œUNASNone?ïöÇ-aÉ/?Få`",R?9ÈÿÖ
@Ÿ?3Pó
†(?GþÊ¥yÚ;?A—8"f£Ò?ï¢ÌdÓ?‡$œv֒?sِÂ<ö_?y•¹¢?zÀnn—h4?€È-È9'?ïa¾ÚaW?}NPØ!#?€Iâ£Øõ–?pkږ}?‡F›cÖæ—?tb!T?ïC?[ú@'?†#.®>AY?Y"ۓ¨Ù?S¦ó-Žu{?•þãL{6?…k6d(5?ïü6øÄê?1Zn¹4?&Lnœh,&? ù?°
á)?3"(ÃÜÇ?)
¼òÍä?ïà@åxjJ?h÷Ó6ƒ?[ù§PÝWO?TôRVà?aÂG
?cHÅÒb?ï¬Ãù¥¯
?k<"-헩?s¢ɜ¤?bª	ÐE?uûuô"M?_0*ۙðâ?ïÙ·Vy?aüMȧ¥~?@ u*?1ÀÕ:'Fµ?qg¢•Z‰}?aYåü(AGN3FGL J0923.8-5154@q=ÈK¿òS;C£À8Íg<O;§À:ÊPrß?â ¸tu7@
GWŎ¿÷@`t	¿ã³íÅ벿ëuÖ?!¿äºáÊ#¾æ¿èÌPi`'UNASNone	?Åñ¯/X?ÁFåÍNÒÌ?°#¦"^3j?°å«<Ôê?趎Áñžá?ĂށÛ?®iT·ù½?¹ËRÔÁÁ?Êp>¨œæ?¿ÛGA¡Ð?ç}[Ι+?Äèú¾*P>?݄VÑÈà?ºæBáôH´?À"	?¥ßc˜ÏÆÝ?Ú2©´÷?ºr>1¥$Î?Ñ3uÇÇG?µOZ%][?ÁY€NïÒ?ªç(˜¥}Ó?ã$.¼·è?¸¯â'N$:?Ú~¡VãwÅ?Ì¿¥>_Ù|?ž.c¹º€­?ž)'
7?áÏ<6Î.ˆ?ÌüàÏÚæ?¾£+jGO?ÐU&'Óì?Èmn~žý˜?¶ˆ:g(.þ?æ>üê÷°?ÇR&ŠÐ c?èIPå[ö?°œ´Ët??²#anýù?š¥^¸Íì?ÅÉèý–*?¬®˜¼q?ÝéÖÎ-u?µSÜeM
?À8s"1'•? 'ΰd§Ã?ÙùïpÌ×ñ?´¬í›ÒÂMIXED3FGL J0928.3-5255@q1MjO¿ötڂ—õUÀ:_UÐìíÀ;<ÔL?ßcOüÒ@¼HKôL?úgΠ·p¿Ð¶*
ðƒ‹¿ïÿ÷Dx2Ÿ?ïþñå,Œr¿½s54rÖëUNASNone?ïZm–ÊK?Ó	EÜ«?={؎X9??‹dO"'ê?"<nHǔá?œô25jµ?ÒІê"1—?Õ´¾ë…!?¦"j½ywÚ?¨MÃvô?å.…Þô'?ÔÎͳ;g?ì8XýOÕ?¥Nñ.õď?" 2ð*:Š?ƒ Ëfl,æ?¹U+Xšâ?¤šŒ]ÆÛ?î'!Ÿr?²Z.á¿Î?)õûYµ»?PJyqÔÀ?¦Óùz r5?²VJÍ·6?ï»,"ÀÒ?‡%ˆ‡Î?7dR1r‹/?9§"½>8?€yÔÇý4?†Ê̦é½?â_ævá?×`zŪ?¥­ÈKnúp?¤çÝûA	?Ø)‡+
£P?ÕdRaÄ¬?%^ð?"ùœŽ—?†g|Aî,±?}˜Ü-˜?©\8~
lÌ?šìí€g?ïºÀ9J?ˆä™í7¸?:9q\]?T¦ ·ÄË¡?€~3ÖÖïÆ?ˆ¸y&ßMIXED3FGL J0930.7+5133@d·—xW)³@F®$‰LD|À:ÊA{ËRyÀ<!¡t­¿ç'"'åw>@îÔ&2n½@‹ù€_
ý¿è‡>—Y<K¿Ô/¼«Âf¿ÝJ@(l¹D¿äÑäª0UNASNone?ïÜã
ÚW-?qG!5U]?b&FOúµ?h»'ØÐü³?`ö¯¶0•?`@ãeZ?ïaê~—^?šæoݞÜC?ƒ¢fé¹W¨?•ZîÍ£mu?ƒâùmÂ`Å?Š5®k@sk?îéš<EšX?ˆóii‡r?ŠØŒ¥h¥s?~dµSäϒ?•`r(þI?µ9É'Ž?ï=±ÃÔM?ˆ]‰eGl ?y%álë0}?r¯Ó#Ÿ]¦?'O)_ª?")ˆ§;h@?ïøm›ÓŸi?J2Ïn¶Žå?5KI(È?6Hv}ŒHH?C£ìåÿŽ²?C˜G|(?ïÖ¹Ü@nk?r7p®¢c?cwe¹pÿ?b< §ýJô?eξȴۆ?háo¸ößK?ï~¡û?qâc…Þ?{¢ÒoÒ·?fæܘÛT?'†¹b?ô?h£'çÜÇ9?ïÜܗù?aΆw\9³?TÿãCìqã?Erœ[ì?h£v(§!?^Ña~ĄëAGN3FGL J0931.8+6739@b%M:'£@CâöÕ®À:ZxyŽaWÀ<:§›ºÜ?´>xt鈆@F[oèEN@T1ÿ¬s?¹hBý‰5Ò¿æ	8Ö`Il¿Þ¥LàÙI2¿á7vjP¼íUNASNone?ïó(žÒ?P½ãK?1EDÐÞ-V?,¿m²»ïÊ?T)¢ó+?KÁ{Îº4?ïi…+ðÁ?'ĸ j‰?€ÿ]rë½¥?"X:Ñi ?"ŸWœêžÿ?‹òPƒ¿×`?ï	ËNƒ¬Ù?ˆ#D¦î®Ù?‰ïºŠrL?~¨&±Žèš?'θñ^ã¡?|ÝXDS?îíÇØNê?•çöžØGÕ?òäDTB?xŸ÷'† ?šb_NLÇ·?"|ïh"ì#?ïûiÁƒ?5bÿŠ1J?!Ý'ù¤)?©[i¤¥'?;ÈÄàè?1½SÍÀ׫?ïÐ/«`¹?r±I"»Áß?eêŒs¾Û?b"Ň>9?j
CÛa"?m90(3÷9?jáäü?tcüÊ°ƒ¼?zL‡llL?nÏ%¢'ñ?~ïCA±á?dôºpäw™?ïˇQ¡?qYª¨?f¼ÑóÊ?S}6›úEL?nø»ç™ü?lЀ,)7AGN3FGL J0935.1-1736@oOö©?)@8²~
ÇÚÀ:#×>?Ö°À;MPëªÞ?ؾ`Èíš"@bŽëjÈ?ûúp™?ïô¡›¬Õr¿åU›d䠿΅.jC<¿Ý
Wna\UNASNone?ïõó|äØ?KÞ°¶~õ.?4²cÆ»Œ‰?2åD‹|«?P«€K:Î?H#3Ñ¦?°dÚ?¥"Ù÷cÁt?ˆµêš¹?bʧ7ú´?'1yµþž?¡IjÙJ†?îÏkð`r(?‹Ð}•Ø?Šá–Дí?~…pÔ?˜¡¶àw?…0DŒ%9?êûbÀ®?°|Gñëœ?'}_Ú¹¨
?'¾`'*Ô.?ÁÁI0©?¯¢m‡ø?ïúýEÌ=?7ñP{ïåü?)ÓÁåᑐ?'='¦ä|Ð?;-V–{L®?1t­cq7"?糧}+5?p4<êä\?u*FÈ4æR?'8ñó%?wø-ã7ÿ=?…'ùÁb?ïm©G¦K?yQ«
[Ð?}é4¡ ç?pyÈÎÌ?…¡o½ð??qP»mJ¤s?îu¾¢ßàÈ?''Pt.•?ŒF•7¬Œ?{™6kПG?¡'"oG½W?P~ÅR¦AGN3FGL J0935.2+0903@lšmÚÏ@D.÷<ÉÀ9àyçLªÓÀ;ÈÓÄ7ÒÕ?õRl>A¯"@׎5bbv@8	cr–¿À.(Q­Ç¤¿å®Wa™U°¿ë™ISþQ¿ïÿÆç'
'UNASNone?ìO€n>;?»eä

\?¸³vÓL?º0ù-d"{?"OxMj?•	Þ×åz[?âÉG>­å¬?Æx ½F¿O?ԛ;k0"?Åo¹Ù!'B?·HÙ»š5Ñ?³Þ}‹^'?æbҝœ2¦?µº9Ëáfù?ÌkY³X:1?²úµô[@Ÿ?´·«'n?¢pGH?Ù遧0¸?¶Á"Ž¶¾M?àû&2×?¹JŽƒ5á?°H5(æ?¦×íùF?î‡èµÇ³Ä?­îm¸="?¤'¦Ýc™?¬d]W?w'·Â.ý.?yù€ÓmÆ?éµáÚ:?½¸úâ"¹,?Ã<
ÍHÏ?º†aê'êà?§±¸
;ì"?£¨žŠ¾6;?êq1L—÷ó?«æýïð8?ÁžLÂây?§:Ú¢Ì"?¤zrPÝî?–|	ôr¦?烹G@T?©1S¿"s?Ï'Ôèª"?¦j
ƒ~µ?–J/ˋ{?'XteMIXED3FGL J0936.3-2114@o³ÿX:S¹@6n¾‰¬½À:`'b"sÀ;¹ö¥ä*·¿ð5§=h@ǽµ'®F?ý|@€M?Àømºm¥¿à
¶¡è´¿×¿Y±¿Ü¾¬3á?UNASNone?ïòљ:N0?Y—ªÜÛ_?+ž€"©?( <±'t3?Vèýü5î>?Xl½ÉžÌä?ï§ðýâ!%?ˆgAR'»?p–
'á?w•h­ù'ú?{qo~‡U?'ˆEä±µ
?ïJ˜ñÓí?¯îDi¯þ?"TŒÝX?vâE2оõ?‰'¬Ö½Z?t®ϪD?ïo§ÓC3†?eÁn(‹g?7Ÿª}?6礭 ü?'¬‰$EHx?3¯Áàž?ïù"r¸P¶?F£+Nœ?  cí¤)‰?éwÞت?Eæ§Ñؒ?EØ»¿hÁD?ïàهxãI?i…òxN	"?Y?Þé(n?Sú	'rÿ?b†‰(S¢g?d&·ˆš©F?B%?s¢ù¤Òù?wÙdæٛA?i* 8?zâî|jJ?h´u7Ž·?ïã<È)ÇF?Yållîøg?Â;KÔËA?Z¥Ä\V†?kÅ&79¹?Y"ÿŠ'ÍAGN3FGL J0937.1-4544c@pô ě¥ã@^']Šõ'À9±aB:73À;A€t.¦¿Í.'¹5@dÆ(Bê@닠\¬S¿í°½wš@¿àMà
õ¯ù¿ßÛ[ž"Þ§¿ÞÛÎJv=UNASNone(?ïãØ ­?d´Ù ¥4€?W¼<}@?W
¦:͕?auºý¤~?\üC@r:?ìÎ5ÎK°‹?¿²"é'æ?‡ã®>‡ñ?'ŸµYÁüà?¶'ÛËàl&?½^	~6šN?í­?EæE?š?'2?˜ûpˆ©1?†%ð­ç)P?¨®{碩?"=¨ùÙP?î'û…µ?–ûžÃæ?czT]?_Ì<¾dd?¬ï;
áI?•ª[É̵?ïö¼‡°8?MH¯FBŠ¨?>"	ÚK¸A?A€§›¡o?EËÜÚP¯?B¨Æ+†DÒ?ïM¿žf?âӈùo_?l\bu ً?pÅ5Ì)ü?'¼ãëp?šœýN›p?ï<KpýÕ??'+£ÿÇsŽ?ƒ2Ú4I̽?rQ	žâ¯?ºI¸a•?z1ÊßTd?ï{	ø–?t¬'…N©?Uéia?BSŒ¸Ëû?Ž€_@?PÇ?s÷wµ_"AGN3FGL J0937.8-6407@qºwÄ\»ÃÀ!"Ê`"À9Ó9¾hÀ;…jŸ±
Ï?Ȑ}l£}"@m¼}cÃ@\Bjy¿âRD###¿ëI"×ã¬7¿ã]W</ŽÂ¿Ú^žRÞ@µUNASNone?îëóIü?§+-×Þâ?J×'m?SÓ]öÛ]? ÕnÏø?¦î±)&k¯?ëù·ÂW0œ?ÁÛÏï0?–>]1)/ß?vºßsõD?º¢ª Ž;©?¾ï&­­'?íLìVÍ8¥?žäÿÆ	¿:?—m•ÕuÚü?'å¡$hm?¯zo§•¡6?š$#¡Çp?í:C»@³N? {ÕUµÓ²?zaóÿ?z¶ÀEPÔE?´‡ÂókXO?Ÿª¶>ÄJ˜?ïõ`6C?°=IÀöý8?>.ý×Ù
‰?a>Ñ©*Þ1?‹ŠµZ}@?°NÆ&r?îÅÜ>kï?«Ó†vènÞ?€­q6©ØR?Š
‡9çú?ží¿'zâ?¦³°3Hˆ®?ï)÷HÚ(?ˆÆî}ê?'<Ý?jNةLj™?'ÿþ,µ"‰?~'Q/pÒ?ï[ìv¡W?~P'gì»d?kñÈZ#n?]	€ýx£?'!Rÿäù«?|
­*TAAGN3FGL J0937.9-1435@o8ÅCk@;48L`À:Kç]qËÀ;¹¤½º
R?ãC^ÿƒ@j3PåJÈ?þ<¶úS?ïý:"£§¿Ù"´¥Â%¿ÚÁlÇS'"¿è°Iۅ9UNASNone?ïç/,Ï}?kç‰ëìl¹?c¼ºy™º?jN< …¡3?DPbø;*×?CôÉ¢5l?î(DlÁ?¯jv:¸? ã¾ÍLýÉ?£5ö«õ:?›"ÝUù4I?¥š0m[";?îՏx¥Ð?'Øz~A¦?"VËѕ­~?Ý1°ˆá?÷E°Bb?"vøteÈ?ê­þÔÂö›?°•`"7"?³Ȅ݂¤?£p¯,¸Kµ?·€@Õ
ȁ?¨#êýЪò?ï÷•&²
C?Q~'goö?GŸ¹3Ü?Lׇ:BXW?4Y›'?:•­B¡ú"?ïTŸ(œ"Ø?–'Ö!¤o?‡S,9ÿ1!?Šy[XÔ?ƒ…	1Æä?žÆ S?ï5'[Ko?Æ§h¢³?‰ã‡iåM¬?†à´½	ÖÛ?ˆ¸!Ê)ˆ?"ú÷":ʝ?î>³›Ç?'Üù¾èö‰? ¥no6~?†ž†~1ß?–ò̽g¼î?‰SïˆAGN3FGL J0940.6-7609@rCóÿ¬*À1lÙÆ°SÀ9?ÎÞ¨À;tOÞd¤Å?½)7ÿD7@ÚÂ-âf@H_•;ç¿æðýlŽõ¿ÞG¿myç¿é›ã±¿ïÿۄ—÷%UNASNone?é¸RWnYƒ?Ç)v™ÂçÏ?DZ±ïÉ?ƌtfü†?ðX°)ÚÃ?™ÓŒÕG?áèªã‡y?Íè:º}H?ÐIZ‰A?ÆsÖ˜T?ÇÊ7…!y?Áà}?äKKõ:Ãå?¶'ˆÛsh3?Ð¥†?}L?´'€hYî?»‡X4°?£ˆ4BW…?à_uM_ˆ?ÀõúÙg\?Ñôrᧂï?Ãz½»•?ʙE«|?µ4kŠVt?ë÷ÊՄ^ý?Áaぼz'?¼¡"Æ4'?À7Lg"t?${þ?œ(o‡bº~?êv܂nÒ?õôÐï=²?¸§#»‰?·«5ß1î?´-tƨ$à?µSwbRR?èû†è«¿P?®tőԅ&?ĉ켁P?ª[URý?®#IÄ庿?˜v³ÿ)?êÁk/pR?©·,®]È?±Z´ïoëÊ?£#Ò(þ½?¸˜ßµÊ·%?¢û|ç§AGN3FGL J0941.0+6151@bïu£KÜ@EŸÝ]=ȸÀ:€º¥'ÜÀ<
±qýs^?Ú9üSUÆ@¾{
L¯@_"ŸèN¿êô
$ù)¿âe U,y¨¿Ö¹âÏÃw9¿è–ËFm€?UNASNone?ïì˜=Lè?f¯ee	ñþ?_gž‡áª?e1©p©AÍ?=ŸÔUÈ?=Œ–"px–?îõ3'Û´i?˜ßQKÜ~?'®¸Ôa/Š?ŒÄÀŽ•b?U­™qNÎ?ÿÛÞ[Â(?ï˜ä_\ÿ?‰졬Í#?ˆ£»ÇÆò{?|žf+?'ÛŽyß?€¹ˆª*??î­»I–¾?—á»íG?"'× 1¿?Š"ÃÃFÄ?–Å¿»Œöƒ?Jϲt"?ïï¬ês?‡;ŐÞÙ?]ƒÜ›nª?†ö¯	Èt±?1c%xA-o?AH rÓL?דּ»"ý9?z(¾UŇ?vFó—Wn(?m‹*`fË#?s_.íe'?rjG퍋;?ï6-[?{Σ­ié?wpH`ðœg?m[jÕÚê?€Bیûÿ?uҝké?RéÔ<?vXY+?è?€ÕQÆIF?j‹m¸fw§?lñeê´Ï?jMœØ›AGN3FGL J0946.2+5209@d7Ÿ©~@GÁÊB®Ñ9À:/þ|rAfÀ<ãðÖ?ä²]Lƒ³¡@ЩIëñ@á'uƬ¿ç/ϓ ¿ç:`ϒi¿ïðŽºå»þ¿ïó¨d@OUNASNone?ïàó¨?¦¹Q.–¢a?jŠµÿj~°?¦»ÈÑîß?C]Y
[Î
?I;]*¡¨?ê"Þ
{Ê?À3†Y?ÀŸ6ä7?º9†XO?«Uþ"ã{?¬Ðr°ê?íü–óZN?–À)²H?ž?¡h‡š?"õð©î?ž6Qnß;!?‹žð#F´£?â"Eû?"ƒ?Àv;#J;?ØZ¥N>ã?Á3,ZÚt´?¦Ø˶ˆ¿?£Y"˜iH?ï㣈'MÄ?¥]¹ôëÀ?i¥}#&€´?¥^ƒLˆì9?5·Ô½ÅÇJ?AºHqêé?îß~Þ¶?¢‹u¾É? €*1×¾?ž{|¤ËŽÐ?iÇw€óŽ?xÚ«^rd?îæ?4H\?†oc«š#â?•c'鯮?€h¹×ñ{Õ?‹©(Hè?yvtµŽ^©?í#zcÑê!? 
 /z?´ ž8ÃH?›ºËdå)\?†uAû–ò?ˆ@‡T~¤¤AGN3FGL J0948.1-3641@p¬/ƒ{J#@)üõ:uGÀ9N]-؀À;"^‡tÔ?얦/ݛÛ@gĹWúé@Æï¿kn¿ç¥ASÈ¿ê÷˜lÀ?¿åJªn÷¿ïÿ²,(UNASNone?în`ùÑ#?¦èwŀË?œÔãêå?šûL¼BÒ?•ZðÁ'"¿?›$Ê=:?ØEõÄ#A?Ç­jö‡Ë?Úsx?#MÚ?Ã1æ†K"?ʍ#ùs7Ê?Ã#\?_Ö?é%wñ~2
?¯;ìÎ̋œ?À&…Ã×c\?¦à¡RÐ?¶‡4í©ƒu? Ro¦Ä?Û4ðÂËA1?¶[œ:?Ý?ÙOYsR¡Ò?¸/2î¸ÜŠ?Æ÷k"Ä9ù?¯åŽÞ¬S?ï?À'àJŒ?˜²Ò2Ç
?ŒM°"d²?Šã2bV?ƒÂ*Ä9)f?ŽÃ«$¬>?äž)'‰!?Ä\'*âˆ?̓#Ôy)?»už4*vn?À7ù|¿T?¹ŸÅŽ_?ìßÂGZ)? ±nݺM?¯TNÖÁÑ?˜*À`iˆ?¢¯öIO?YÞ¼»?æç«3[2g?©–Ц?˃¬C%ªÆ?¦JÅí|É?±»Máغ?™1`—'ÏMIXED3FGL J0948.8-4243@píƒ<`Ÿ@ û¼ÓZ…ˆÀ9ª¨ëF4˜À;u­Ñ_Å¿Úç'euz«@
;R'rY@ñ…@œ'h¿êeÜVòD¿ã9¾dv™‡¿ß0…_a¼¿ê(,"dËUNASNone?êä'ñ¥c?½'/í?·"jBD¸?µ $ži
ë?±½t¤0/?°¡Èèì±ý?ëÀ¾¹0/??ÁR'ü²?›Æ"w¼g3?ž¦UnæJ?»e!xº?¾j"ˆ–$?ꑒ=s—Á?«ŽÜR+?³''vs?ŸZóNhY5?¸KЀ¦ý‡?¢Ë]inG?ìLæÉ´P?£öºø] !?'y"¦Bto?…á-ÓmÖ?»7 !Àg?¢Ô?Œ Îñ?îëð4õ™ä?¡q[ße/ù?",tŽX"?"%þ<<Ž?Ž«	›™ªà?"'ìJnø¬?î㧐'U?¥ŽLÁF(P?'Y÷]f-?…᳎¸?!?š—Þ°ËN?¡¥	<ÔB?îJtM.Üâ?"²9xœŸ?›•é4,E?‹Ô	é"f?›1àwÏoi?…ÜeD´W?îޘ•sÖM?…¥ÍMˆñl?z¶Zœ"?h©z:ÃEF?l|Æ?ƒÈã ZÅAGN3FGL J0950.4+7550@`í(Œç°@BD–Ý&·$À:Ö`"•À<=%ÑJàÏ¿ì1Éc‹À"@
óp˜nv@'Í@¿èòW‡´¿ã¡ãÙ?8¿Û™;‡·ç/¿ã¬¬
VèfUNASNone?ï®P®ÕQ<?No•2Xw?{äˆ1'¡9?Š›.ƒÆՄ?iæ@Ÿ®	×?q)›¨À?ï–õÓmŽ?‹§.«Ú¦å?vŠ	⌑›?~`.c'?}û†;s?'{H©œ°ø?í¸‡Ú:¯º?£È†Ï?©5G;|"¨?¢~¼ç…'?–"vHûV?ñÄæõ/?ï´2²¸W(?w=õ§Yô?NssÁv?JçÙb›Lj?†'?uâxEº?ïÞ½-P"á?"u;Ž
^?ikÕ{?ƒ7I«¡?O^òV>J¯?ksÖÒ³?ïÞ}5#½
?iÁž8ì·?]8ž°Æc?V]œã¯ù?bó®JòÔ?ctLd{å]?î'C0x»?š	A2ª?žÝ¦¨ É?šG‡\4?¡gôNÿ"?hû1Å¿?ïô…
!?O1†A™n¤?.8é5M;µ?!	ðti³?S.Ø<ºîð?M ä~[AGN3FGL J0952.8+0711@l·`—Ì@E¢}sÉÀ:sÐIYÀ;µ™9øI?Ô£xM¢'æ@
jT»ï?û0©ôg?ïùcñÁùµ¿ ['îËi¿×®k@sk¿Û~ˆ&ÌëUNASNone?ïï?*¸:o?Yi XSÁÝ?CPömÕ"‹?D'ŠÙ¬ý‰?WÙ/Ìpø?S+4'CŠ?ïP
y«'•?šJ±€ËTm?"fÏVç°º?Šw¦d40T?‡–'J'AÙ?"ôµt¦…?îã©KyŒD?‰K|º—"Q?Œê˜Á€´?~4ºMŠK?•Š3}¹r?Zð>?íA[ə*x?£ùé\_?œIú=¨•?"™ÉÝ\¦š?­Å´kâ96? ÍBs°
{?ïøø&—ÄW?DIà@,é?/¾VN2s;?.5'¹vÝ?D/Ï·žùf?@nÔQz6?ïǞmâ?³Ì—fE?kTK΋ò?sU1ˇ¼?mVŒrJev?tXüu£Ç?ïj•åQu`?}U°)Ã@?€%û¨/œ?qt¢…xÀ?…4‹مÝ?v=è¢"¬?ï;É´‹Ú·?ƒw öu3?…¦©àT7<?r{®0±L	?‹féï?~ÊèEufAGN3FGL J1002.0-2837@pyæ{_ï@5¸Ç\J"À:*ˆ«€À;µØÿàöO?çÇ(¾Žñ@GP×3@œ	ßý¬?ÇVùÌ_>ª¿è`ë'UÚR¿é!ÉÔIï¿ïÿB¸·AUNASNone?ï€cºån¯?*ÏÄm?ˆô3bç?ŠÕh…jU?kËw³MôL?l®‰\?Øytjc?ÉÝÿ"ã;?ßÅÑjDw?ǟ"‡
î?¿¨†F€˜?½Ä™]Å¿#?êÒS®öš?¦l6Fÿg?¶Ü—œÉŒÂ? sº¹"-'?²Êìπï?œÏ§ÔÞ?҃
¢;9ù?µ3ÔóÓ?âYZp3?»Ÿ÷Ÿ¼Ñá?Á"zý2n?°]ç5¤?ï½#×ú?|öRª	·?y… ò3"¿?z 'V`?_¡Í…'—?Z§—ö|?åsg¦NÖ?ÄlŽòTNi?Ð"ªƒÕ@?Àó—òz†Y?³ß'¾4P?´Æ`àô?욠g
Š?¡2ÓrŒ²?²MÀ Qk?œÔ=hóé?¡»Ðñk…?Xûlb?äN›ÑN´?°›"ã¯å?ÓD™3Pÿ?¯.ÿ	‹?°x½O(?žÌl&LfMIXED3FGL J1003.7-5215@qlKƧïž@–ÎãþAºÀ9Æ)É'%ßÀ;7]ig¢§?íb¹æ±6@˦‡Ù@{>ŸÍæ'¿"±h~Èô¿Üþ?FοåµjlÒ³Ž¿ì•h.èuËUNASNone?ÊÀØDF£J?…hý?踼ܷ?Ã?îçm¦»?'á¢JVá?—CQâ–z»?àÔBd¦?ÐðúÀYŒ?À«RÖš?¹ '¸'8?ÖR3î2è?̈±z?á?tËY?µAk¯¹\&?Օåhä?²îh¸Å½?¿¯˜Q£"M?¤²¸ÖI?ái¯sþÄ?²×"+"?Ìêœk†
ñ?°³…
èÓ?Ín§8Ï»{?­Éì¹r–?Õ'2`pi?ÇÂ~ïc?ä'ÅÖt§ƒ?ÈjZÊ%þ?›4#îÓ¥?§'7ŽrÛ%?骖»?Çìn¢È†?°Á‰¾(pí?¯ÊSޔï?Ã,'Ão3?Á¥R³3Ò?æËÜ.¿†?¯É®ºX"?Ì+/Ìãô?¬Ïp±'?±P»¨	å?šv	š1?èGIP^›?¢ü"²üvq?ÂÀ׶?â´îô9Ú?¹©Å‡o[¿?˜Ëâ֟?"MIXED3FGL J1008.6-5706@q£*\|Ù¿î3†_€>À8&Ô©À:(ÇÅüÎó?ÛbÕh¸âE@
Ÿµâûba@ˆ€—•¿äúEoº'Ñ¿æy™¨s¥¿ëAÀáÿ¿áŒs%¡UNASNone?Šz'Áˆöß?'°9z<_–?¶ÊL8¢?¾™ÁÕ?ì¼Ì2.a£?¿'FŸTL;?²ûž[ˆ,ƒ?¸Oۘ>;?ÁÃ; âZ ?½µ¤_=Ü?é/½LH¥X?ÃÎyäâ1'?ÁÜC§
O?¨"XÎ>?ѽ™©ø?ºY%ÏâÕ?ãIh°?º¼ä'Ãz?şnÁdõß?¸ì-Hå+{?®_<èö'?¦WÞSÖîn?è²0}/?»øËvi€?'=æ÷b¥ü?œÙã¸V6?³Èd[ÿm?¼×Æ1õgî?ìõ
{Ç)R?¾wM¿P?ŸP'_ÀZ?ÆWaJ?Á¾ûÑ¥­,?¸S.ß¾ u?æèmHþ?ÉÕݛëÈ)?Ï&nsûû9?±!d,§S?ϸ¬Œîîé?µ"A¤…Èç?àH9?ÅEx?¶‹óá½	?ÐnØ÷cµm?½qAåíI?¨izaØӏ?"õÓT›û®?æAûÞÍ ?¾\ÈFÄú4OTHER3FGL J1010.8-7645c@r`ï~=ÁÀ0¼øµˆãiÀ:¾7ޓŸÀ;o	µ‹g¨À7º¬cˬ@õ&Ûa:@sð?m©&¿ç–î÷ø}¿ê¬kÉ°@X¿åÖÆ]xÐ?¨ž€Íߋ/UNASNone ?î×;Æ.è?©1̨Pé?T"b°ð<"?WqÞԉ/?¡ë;'?¨ð°-P?²s҂?ÄêçPAó?nD"ÎG?x5{e½¦??ˆB=`_q?‹ Ì"Áé?ìåD•4? Í7J¬çù?œïøq1?ˆ­i…)Ë?±›IÖýl?›€Ö­Šâÿ?ï€îŸQáÁ?‹c_Xm>èÏO,6J^>ù»•EÑD*?¾$U"GÌ?‹}©©ý­?ïÈ`,¡¯Ï?…ӝ^±€??n¦O±2?D²ðÊÿv?yØÿ'kh?…ZÇNja¡?ïÕæ\ÑùC?s
0o†c?Uøè®Z"ñ?VàYÑÀm?o/4K?nRv«<3)?îû'ùJð?"£ƒ^aÊ?‡–jšeŒñ?r­®ïU.¤?"Âk"dQ"?¿>Yø¦?ïéWKìV?]¢Ï¼V&>¼¼,LÐ>¿«H¥–S?f¥mÃíø?]¡r¯¬¯AGN3FGL J1013.4-4008@qRÇ%Ä@*µÿÅGÀ:=©µpµÀ;ª\™'6¿àvÃá@3%>Röó@Æ ‹:Ü¿ãM-M:¿èw/òêv_¿Úzƒ9L¿Üщêc®UNASNone?ï~wÐØ0i?¨¯t'Lî?`7Ü÷ý|?–[—€Æ¬?ŒTŒüh¡?¥û /:ú)?îæÀ l8?©Wx ›X›?y`L…çx†?"eó>ŒB?œÏèÌaáÕ?§,añ?íþ¢Ç5‰?œ$4áµÇ`?'T܏Þ:ü?€_¡—g)Î?§ki½UWî?—âŶis?îíGND^?‹È–!j?Pæ…M6à?Q î¾ãJÖ? ¤Vð~b?Š¥û¤<?ïØ-Âʯ?ÄO(x*oQ?'r¼/ýè?¾YšC@O.?Œ$|@€>M?ºÌ]ë\s¸?ﶔ«ëx+?ƒuª¡0Á.?b?¬±I?ajö—/p?{–ýõß?€‹UÍ×?ïN.å×Æâ?"£šG– ü?~‹`)a&y?p1Ë°<PB?.–nÖrI?'fÊl¦Ã?ïÇë`®
?d x|±µÿ?@#–BW)'?1±»Î??zÜîÄøz?cÎNòbÅAGN3FGL J1016.6-4244@q/È÷Q@'%WšñˆnÀ:#ÜHjÒÝÀ;'Uœê†ò?á;Ó*½@x|¦CÌ?üƒÒÀVǸ?ï±jØÞJp¿ãæh4æe¿Æáâ	í6¿Ú0âÿ$tUNASNone?ïø¦««4?HøLo\o?(óÐoÖ	?*:v㎥D?G(`¬ì?F¸áx?îŒBfX=?²·Ù
?'g¼
u&"?ý?ôF??¢¡ï²ã"%?°Ø΍T,v?îõn;X,?Ž—v£ææ?†ÅW'¹?|^‰´),?•ù†ªƒÀ¢?ˆþv´¼ë?íÜñm@U?¢ŽÜª¤ÿŠ?s"é½è"?w'¾Bò"?¯Î6'.?¡÷Cicº?ïüÙÎy0?3Þ6Cøõ? ³"µù?–Ü>"¼d?0×ù±V?/­‹œ1u­?ï™Z6­;7?V2Òë=ß?j…ŒEs?jqû‰¢ê?ƒ>D‡ç?"vÀÓ?>4?}Tƒ<npû?zŠìøöP?rºy^ Õ9?'T7¬íóß?t‡™Î²ÿì?ïrúÛfª?€¹G$ÒÖP?p†Ï¯H?b¦l±q6*?Šþ…}vÜ?~E"k%Í£AGN3FGL J1016.9-2653@p"æ1ø @8sÀµgUÀ:ùã†MÀ;ÁSL®.|?äøã#%t@F,6ê¢Ì@×(Ÿ[zz¿äšèù=f¿æ
Hy&Ä¿ê²!óR¿ïÿå|WO®UNASNone?ïŸÓðáÉ? ÿ8§2Ö¹?hrn¹©?maJ¢|‹?îh.6Ñþ? "‹àõ?æö‡çsä?ÂFLÍ}?Ê4<¦,-?» "Âf¹À?´XK°…?¶që5z?ë÷ÉG²F?©V%ÌNj?ªd'8ÇÔ?"ë4'BÙÒ?³>{øƒf?¤ÛÁã2ìq?àèh°ÝFÜ?³ç^íååç?םxšªø?µoŸeA•z?ºF×j_šD?¥16'×X?ï½>ܔ?•:7)$ "?\»\>ô¢I?jyó"åjr?z2qzµŒ?'äÝKs?í´¿ÃX?®±úd/‹?°°p6#?¥›ÇO¹Ó?ŸIç®@—?¢î§¡›Ðé?í×ñÝ8»ï?›ÚÙ]‡x7? 8'
{`?‹#"*2"¹?¢}©šŠÞª?–_bså?êžꏼ‡?Ÿë{ £1Ë?ÁI8M?›âÐÆá¹4? ùxcè(?Ž÷of(ùªAGN3FGL J1018.2-6254@qç"ßÎ1QÀ'C¦GýÆÀ9–©$Q!À;A#·;k?='9@)ÿæ)À@Š½¿¾œ]¿çXQ¹—L¿ì¯ \†ä¿Üi"Ei8¿èø²JYYQUNASNone?æ—ÆÝÛ¤?ÆßØÍáõ©?¶+"iµ›ñ?´«áýðã?ʎ+¯ä½7?ÃÅþ…	GZ?ÐÄïVB4Œ?Î]¢Gq?Íû‡Â£öa?À¸F'l$?à¦d¿X?Ë>[¿]<`?èbbIºøÔ?­s4lM™?·3g{›I ? ÐÍá•sÕ?ÂÜÃëea?¥²•pï¥?ÛKÆz^?¼Ì¢ìÆî?Æ{û¹tUg?½0¤Åi"¦?Ùw¢';¬?»ç›éÐò?ë|èw¼éÅ?¼Ø
G¼,?§rŽ1ÄcÁ?©‰žº?×[?¸_u)6û?µŒÝÊP9·?árx€ä±?Ñõv¦ÇÌÕ?Ãiˆ ´&I?»Ý:ЂÜ?ÓfK'¤#z?Ë­T'¹.?í(‡XX©?ž™<ˏm?£ìHrr?'£cÄ`ò¨?©ç¢?tMô?"pÍ!B?ãß3֐	?³¹ÀfÉý?ÊÅ˂0,ª?±\€£×Ë?Že#£Ñ´?ª^cÌMãóMIXED3FGL J1021.9-5815c@qÄó#x«
¿ìùcÞ÷œ¯À8‡7ø"Ñ´À9øîº]^€?ò¬g|õ@
pò\ÔA`@iŸè=A¿ê¨ßp¤"¿èPÒüøʾ¿æ?˜°ªF)¿åX£7ÜUNASNone1?vÎÜʃ_Þ?wŒµ¢e"u?¼:4.ZÜ?¾õKËIXÓ?ìOÚÿü‹=?¿'ÁÀ"O?²*•röö?ºÛ'eS"?Åßw{þ?¿èTg?èBæsßB=?Å{	¼þ^Ñ?ÁX^}†5?¦Uí\å3K?џ™ªØӎ?¶uë±TÑ]?âÚ‹2ø?·}íj	?¸å§žmí?¶g_ä¶?²î­ÜÂoC?¯Ð"@d8?ê…u`\êš?¾\¼üA¦á?fe×Uªìÿ?g¨ŠÔT™?Ĩ'DP|?ÄÂÃIr®?ê¿y—ht?ÄÓÜù=H?¾ç[2D–?ÂÏÌnᒵ?ÆRëtؚ?»Î±öª
R?æŽY¼G‹?ÇïÛ¼÷6?Çß+"‡X=?«4—O$?Ðg¾)4Æu?³>‡ÂÅ?áÔV#M7?´ØqV}'Û?½ªAÔÙ?¹{ã¤uWÕ?Àåë#Fy?®:ëq$Eà?è;Ñ<ü"B?ÀÛ'a ‰ìOTHER3FGL J1024.3-5757@qƌ½D¦¿Þ)VÍÀ9š‹1!
À:.Ü:(ú¿Ñ>ø­jÈ@ò¿[Ëñ?þSé Àiè¿î;[¶4/¿åW#P?Å7ÿÒø0¿â¾ôUNASNone?²]¹Žz®?´aùSWYÈ?…Ûä,C?Š$§g(&f?í_è€á‰?¶y®Fï?ɖ_r¬Dí?Ò$¤¡w¬?¬•)§¬w?¨Ÿ™½õ§3?çшõ©Ý?ѕ΍0?ÑØ&>¥z?±i1•ûà?À}VB?ªõƒž\VU?ãr4—P-?³ÿ,¬—‰Z?ݩƘ?Ð;·)?_Æ5Z?m"†ÎDä?áa¡èj¡?ÐdH w'?¡j"§'?¥aw€'¡?"B«]%Éã?"¿ÈC¿8?îÁêˬ?ª"÷MjF9?քéøñ\¾?ÖGã3k'J?±fþg©¦e?§Ø-'Ô@n?␫6­™´?Ôt¸Æ|óé?Ôáy…Z¥ñ?³€¶ø
é?¾Z.ìô×Ð?§†ÄLBN?áÃý_´
?³už@ŸÜ?àʀÔ­?É¢4ú* ?u_€Äb§?mî")U¦?ÞÊ^Õż?ɖßހ(MIXED3FGL J1024.4-4545@q]¼ÓZ…ˆ@#®šõº+àÀ:dú:þÀ;­â1¸ß°¿Ù	­Ä°ú@
CËPuä?ÿmVàa!¿änkͥݿèëÀJˆdh¿×ÄöCÏÊ¿s)â4d¢UNASNone?ïáLó?µFl—7?<Ó±§d?<B¦Yòæ?œ³g1M¼?µE{ax«?î¶E_¹,?¨¨\°ÿ¥?wH/I9Éì?~Osx7?¡µÅÀ±9?§`³¯=œ?íû:ßWœ}?œ&|ê¬ô¥?Œ(
:P2ó?xSÊô*ÂË?©BNº:]{?™<³msf?ïb‰*>Jœ?†æ&A§?1w«ZX>?@¾Œ[{p™?"hüKWû?†Ë§¸à£?ìäÐ
ˆ³Ý?Ñ°EsÒw?)#áÊH'¸?*êTž'?¸Ìí»Ò ?ѱ.œÜ«M?ï©M€*K?Š8^]†Ør?aPÄ%üÄW?`êÒÉ÷gy?XnülŸ?‡ŒVt‡º•?ï?×̸³n?ƒ¦IÑhf"?}\Ō"]þ?f+jw"7l?­ÕqÌ?;áÞþçË?ïä®Ò­?\¼…¹á5V?"œ6Sõ?"ój.W$Ç?j'¿Hí&?\2•÷`ÃAGN3FGL J1025.1-6507@r#9ÀëîÀðÞ	52èÀ9g½ò>v]À;OÅ?é$?ð1©J¼'Á@¿r/r^l@Y© ¢ÍJ¿ä48/¶é¿ç
Šån%Å¿ïõ2\¸"?ï!¦mèfUNASNone?í§€ƒâ¼è?³ý½˜lí?¦}BÆ°h?«©i
ÿ!?žiûo˜+?£³©X\2?ê9†o#?ώûIџ?˜À"m³Ïµ?¤BSå"Ã?Äáõ†‡ø?Ìpv"/"Û?ëÒÔ´Þ՟?£±D{Èñ?­(öË!Fº?–‹ß"L>?²ÔÞñRî-?šˆQë›t?îzd¾#D[?«»¨º®C?r³®uK??'Ò œ#Sñ?¦>NÊ\h?ª4^"Ú?³?ï-ªü * ?¤°'.$ýý?`úÛ?¡¨×‰›?"_%ƒ,{?Ž0Ù÷³Î?í#@9+ß?ǓƒÂ(Ÿ?Œ0×:g›?œ¸ˆêp?³_ãP­þ'?ÄÇ+ß=#?îLm9û_˜?"|ú?˜ø¯Ãkhó?†ÅǪ6€?y©¿©ñ?‰ûûÈê"R?ïÌ^è:2ù?ƒÀ3ùåY?IÔæ'̒D?k°õ\·0Æ?v•ï›"€?~'¯8À¥AGN3FGL J1025.7-5659c@qÁ;÷'?ÜÓ¢©ã"À9·
èaÀ:O|N/7ü?è
j®–ù#@U¶öv¿O@'Ÿûž¿ã]+Í}¿ë@%§ô¿êöü²e¿äZW'=°UNASNone0?¡ìWÇ08?°ÅJ¼˜ k?§ˆ}¦2ª?³ÅB½b…?íhº²™M?½\ï3?²"å‡éæ?»´ßÁ;?·Åõ±â)š?²F‹Ûüü§?ê´Ä˜ÔU`?ÂU´BK?ǤÁÒ)?°_¦@I…Ö?Æ Vyo"?²¢áO—Ô?äxyc²ò?¸éŽTàæ?Îv•
U1?Á®v†_M?ª.—!'!Q?¤­ð†Ãܗ?æ¿qG@?Âw.•e?°MDa›àÎ?À0€è;?£…=‡ä?´7ÈWë3?ì½ý ¨?ŲèH‡?Åř@í?ÍÇ֘Óv?ºÎhOÂ?¬Š{ð@ŽH?çMÿâÎÁÅ?ÎdüÏ
Ø?ՈÖáM¸?¶•¼³Å¬×?Äåêhq·?¯¿>ø@÷u?àyzrëc?¶Öý•¿è?Õêcù+Í?Áu5ÀØß?±¹÷-ڔó?žëè30b?âӏ·{?ÁŠA¾nïOTHER3FGL J1025.9-5930@q֍"M;¿úûh÷:^¡À9õ@‰]À:vc ¹HŒ¿ù\·%Eµ@`?
1@¼¿Àéz¿Û3_Œò0"¿åT]/¹‰­¿í\ºPüпÏeo+ÃUNASNone?Áõ7kyœ?ÁÅÝ$2å0?©î™\O9¹?±z²tm {?éãȏ%w^?ÅãCÇ* ?â.c¢´?× ñé?¢¨°Q°»Ž?ªñü	ºä¤?ÙMÏ."€`?Õø	å9³³?ÕDUos*o?·´»k_ü=?IJjôž*¬?­$Ø\?à1:‹à?¸ŽãB'c?æØpÁ"
‹?Å9Ì ÷¾µ?Jüj£§¯p?W+HØ\à?ÒA HàC¢?Å6Tß?ÒÓzÃb\?ÍI]®©B¦?¤+§wq´?ªŸ«ˆWÉ?åS'ƒåA'?ÎnQ»Î;§?ç.=ãÃ"?ԟô:·?Ÿ̀Ië?£×?½®s?Ïf2La
:?ÒÏûIaô?ã± ï×ÇZ?·*8ꀇ'?¹îaÝj©Â?£}öHBÐ9?Ò!%¨õÆÛ?´"×!CÚf?ëK'H÷É-?´Mہи?$ÈyæŒ?#) ð'¡l?ÂÎ0¾Ó~±?´LfL²'–MIXED3FGL J1027.8+8253@_øA [À@@e¡"úÖËÀ:y¤O\_À<çCp˜?Ó»v«Ô/@
ܲ6žw¥@•¦_Р¿ã¼Ê}+¿Ùw£—–¬w¿å臿Û<÷"œô(UNASNone?ïÏs¤·Z?tßÉdœ'Ž?f'jñÐ?n%çC9Fc?j
}PŒ`?e‰îãÆa?ï@Q0õk?œ­ÙäÚ­?†»Ñˆæ?Œô$ðôK ?‰Ý®
X¸B?"Åç«Jq?îÁ
õÈf?Å!¼üÕ?'ŽMo¦T^?'æ"#\L?–Pp.1ç?ƒ&WŸÒ'i?îŠbb±â!?˜¾µz#FQ?"¾Y¦ì;É?¯#	=˜?™õZN?ý´cXñ²?ïñÝmâdA?\ íºò@?Aý{K?M>Îˤ·?SFUžõÓq?Rvxaûo?ïɗ¡zl5?zÕzÚ©g?hàX…?h
6y¶'µ?m¤½Û'<?t]¹­Ùí?ïl0xKsÏ?xž²µÚÏè?¥Ë†Dµä?o½U¨Tz²?ƒNhî@?n«¢è›2?ï¶>Ð(?uR..'=È?t¼5"žL™?fÔDÙÚm?p$ÃH\—³?ka³"& AGN3FGL J1028.3-7419@rXú$‰LDÀ,=Žc|À9ê)€,À;X¸þ¹¯¿Ê›IÁƒÝ4@OFǏ¡@…:Ÿc2)¿ä¬Ú¼N¥U¿éÝ\0F]¡¿âHS‡Ö<|¿ïù۞ÕKTUNASNone?îê‡Á¼À?°­Áː,?r	6sÓ6?qÊ7=NU&?ž/'õ?œÔà«?è븃GPT?Æ$f°Oœ?¸þeÍOh?µÑ"w?¿£ÖÎF÷?¿Ka°Ò£Ú?êåœäÔ3?¦	™ºY`L?±€Š´•(?–& î:šV?·R•8Hâ@?Ÿlªº?æ:#€žÝ?´:‡xJb¦?µhð OZû?§rÎD?KÐ?Ìbùì·ñ?±X}ŽR?ï†Û—Ñÿx?Žs%ÖB0@?c9š©q?b—¶]Ô*?‰z³l¬æ"?‹'ïön"?íÌRÒÆòÿ?²ž8‹þ?72^>R?Ÿ—§Ëb¢?¤ŸJ½ÑLÝ?©¥.¯­è?í¨4J%z?•³H£/?¤,Ѻc¶?Šü&|x?¡Oé©$Ç£?‰!ìuî¥?ìÇêÓ?›uÂ`?žz•é¢S?‰ÞóD?²!åÚ,4P?–ožvâ°AGN3FGL J1030.0-5809@q҂ýuâ¿Ï¶™šróÀ9žü¯égÀ:H?³t63¿å­¯è)cj@Q>kµ±?ü­9~ÑÂ*?ã}M\¢¿æ_µj¿ç«®TÅ1ֿјšbŽ·áUNASNone?¡U‹"÷ˆ?¬" 'uý¢?'Ki÷ɲ\?ëb´â±?î¡yž–Gn?°ÒŠz7–ª?Îwhy2"H?Ò™b?¦4gN%¤?£NW¢rµ?æþäK?ÑÀžÖšV?Î[	4 àO?°ÞN"ÿJý?¸2%à
?£c*íu?åbøöÔæª?²ª«D'ÕU?áiÜSƒ?ȊRl€Ô?Vðüh"~?]Ð<ŠÌ)•?ÝVÇj•Ô?Ȇ[õóÑ?©¾œ¦q÷È?¹ÙÕ´Rª?'-iڌ‰?'‡þ˜u"?î`Ž`*?¼'»¡"ÇM?Ö}'´Åfs?Õü"Õ;Ô?­L —?¤ñò­)¸?âìt¤[ƒM?ԃ·Æ'…Š?Ôq\É7?´ˆPÝ°MO?·ü/@–e`?¢²ÌÎ'ÕW?âðÁ"h
?µ¤±òù(Ã?æ"¶£7?ÀSDNþ.³?LJ‹•"w?C©p.Þ!?Ó¬mt€8'?ÀP‰8*%MIXED3FGL J1031.4-5855@qÛXâe,¿éôّmäÀ9/Q˜y*À:^2»>/?â,ù|rE@
­o‡l@®<_Å½?íc·yBP¿ÖËïΣ'¿ãPÊs^Ïø¿ÚY°~7UNASNone?Ì|ŽË#C@?Ljû؏3ö?©	€½Â?ž(2ﮈ›?çó")JÒ?ÉkwrRX?¼Kô½¤?'iÿøô?¶½}¾» ?³ ~ûˆ¡û?éžîñËðë?ÅòÇÑCÃ?ÚÙß6~8·?ºùõœF??»ÉÝÑyQG?§ª|?ì?Þ3©T'8?»Ÿ¬e®N?ւˆÈˆfä?¿æ'ï×÷?ªœý¬\¢•?¥¨"ûñ?ãëÀ¿¥?À±ãªfz?Ø¢W"xÙ?ήvžJ‹ó?"ºA'¥x?–Iþàå?ãjN¹ˆ?Ï	®A=ÚN?ÐiB¦e&m?Є"f#þ?¸f8ðÁ²?«òì°½¯?äÉÑåæNS?Ðx
es³?æ*B¶óO?¶žÏ÷Æî?±¨pÖd¢­? 8¡õó1œ?΂¿&_Ôì?´ìgQ
™?àÌ­Þ}¬Ý?»jPô½³?§Ÿ¯ô?•×J€áú¢?ۃM!"E?»ƒÉΕ¤ÂMIXED3FGL J1033.0-5945@qäîcŠ	¿öÃdٞlgÀ85׈±ÙÀ:k qäI?ᬜg`@
*l!à@	ohی¿Á žXùžð¿çe2´³%‡¿èK4ì=Lß¿ê­ò$'ÛUNASNone?®BÚ6¡?¯j/­Cyå?ڙqžƒ[?̇Éëúm"?àÒӝ™Y?Ì«Ñ»°+?•Ø?LÕ;?§éâ‡I4ý?ÓC^oÞŽ?Ã/	/  ~?寎Њ=þ?ĕx'r¶?Êáê¯ûu?°ÒfSl?Ò{N·ü?²F&ܶðZ?à@ ~G%%?¶Lͬff?¶n<5ÊÄ?§æ"†¾¦?ʈ‡Ÿ,fÌ?¶†¦¤yY?æ›0P»ëd?º^4åK/?Ê"ŽFC?Œˆ÷y¸?Ùô#['e?ÊJÙ¾³ë'?ÙìAÒ]Zy?ÉÛ;~Êúÿ?©ZÌhô—?µ['ö~œÊ?Ò×Ê]B¤?ÀX2UóŸ?å$Ïd¤?ׁÎöô?ÜBsX£kf?·ŽcbSpæ?ËH:4þÄ?«È¾Ÿ]^ó?ÖoV•8?µ&§ɔ?ÄTZ–(1?²˜Qò›Pn?Áäb(ۆ?¦hÏnµÝ?æqÐô"?¶¤VZ:ðMIXED3FGL J1033.4-5035@q›—Oß;@	U./¾4À9TãqT2À;_	ðCÊZ¿×QÏO!êû@¹ÿ´€¥­@'À
¼Ç¿ç³ÜæËQ¿ÕP¾Î M¿ÚLfó •ï¿á¸äÒAUNASNone?ﺀ~Ö?xZ˜aô±?Z·Å¨*2?S«8Þ±çD?|ϲªr?v(uâº?í$h'ï?¸\ü1F?Š¥#{à?(?'§Uœz?³ˆùyz¬?µôÀTƒ	ì?îCƒuÉci?•nÆdÜV5?'ô>ж=?æá}$˜?¢M©šnK?çý'üÎ?íÈޖ¬\ó?•µÚ-ÿÕ?s@€lŠ4?jyn''?°…
4o?•IѪø?ïçߪA~ó?…:4cœÍû?EíM;ÔÊ]?A9Ǿ¤)˜?b¥eƒe?…%xåñ—?ï<žª-C8?ž÷˜Ûâ?rL+7Hd?u,"µö?"ÙïÉ ý?šË߯¡š?ïTÑ~Ÿ?}øQêI:?äyâÓ?oËÓ©%i?ˆçE¼%I`?uY£'cá?ï`u\è'?uˆ£Ó[h¦?`3Տ%Ò?Kçu|ÿ9?'÷vœþù§?t§;%—"AGN3FGL J1034.0-5731c@qÔ·éùr?âQ+6¯ÆÀ8‰Sԓj«À:m;Ì^èÄ?ñ7œvë¼@3Qƒ«E¾@D¨ƒñ?ïþoïÒ
y¿êBpI³—¿åMÞzýªÄ¿è´MŒÐ³aUNASNone0?Ãpö|"·?ÁH;ò¹4X?ʚ‹9¸0?Æâ²á­ô3?ä}'ŽÚÆ?Ì©ùu!?=¿c›Y?§9ø¯Š¹Û?Áû¯/ÐI¦?¼	ËÛ¶µ?ê—&;—Ê{?ÀÙ¬CÀI1?ÑXÿÙr*H?¶kTÐ'O?Ƹ8哆õ?­Aƒ5½%?á¥qÙâ	?·Ï' &ܦ?ÃxS?9ž?°B¤oík?Á•¦~ô«?±oٔ¢?漏Ks,.?¸}ëˆÃ&?Ü@‰Ö`§é?Ìc¹ÇPP?Ékùùõi?Ã[dc?×	y›¢]c?ÊèöcŸÉ?²¤'.?¼
F5T±Ä?ÆáÖî'ª?¹íú{ÔD?çõÊ87Ô?Å·—¾D–)?á±×¸…n?¸n,û@«?¿npÐ;†?¥8­dŠj¾?ÔÀ´Zåÿ¤?µàjíÂbQ?ЉÆ?{?³ÈݶÌQÊ?Ä­<Iîr?ª¿}íŒM?âµqÞV"?¶ÁÕc¦MIXED3FGL J1036.4-4348@qjÚãæÄÆ@)9+6½+À:(ÇàÔÁŽÀ;²Y¥Ã£?Éx§À'›'@
‹+ÅUµ@6èßÒãè¿êbägYfµ¿Üõ>.þ‰ø¿Ñ2VG¿ïÿß¡ï1.UNASNone?ëEp#ËÙ?ÁêäÐN·s?²mq¹%²?²Ñh+d<(?³g{r
ÏÒ?»ªãƒrÁ?æ'ÒÔ©e?Ê @O®òz?ÄÑÁ$Y&?À&«ýì¡Ì?Žó‹±H?À<ÄÎÈòÅ?æù:RÏ?³ÑÃO?Æq_n½?±'=Y€8š?»TÈFìp?¦ÎYÞ¦e›?êsϛY–?³û'öµ–Š?´LŒ¥´=?°}Åî˜@×?¸a6š;˜?¦¡ˆî
Í?í2í±&†°?»¸±G¥?¢ëÛ܏V'?¦7°–Ag­?©åIt‰€?¸J`Zw‰"?ì*RRÌðM?º–ö	kR?°‰ÝìÂ?­àRzF#B?­WÇsl±?¯4m+7Í]?ê£Ô¶Ù£þ?©†¶HkM?¼ÑĔ€;`?¥K.˜ííÇ?¬+ieI[?™¾J[¡o?íÿàä~<?–²&7µ—?¢ÌâÂé…P?'8üÊ??šƒ^]-è?…ÛóR¿âÑAGN3FGL J1038.0-2425@p¿á2µ_@=;qdÇ)öÀ:29Úí!À;ÇÏ'ðßÒ¿ôtÞt"ý@PÓw`ߔ@,\@Gù¿çO•ßR¿ãlnÌ&J¿èøʕÿŸø¿ØFc]˞UNASNone?ïò	—ÙP?X¢-—]ï:?Pº,˜?TÑëÑ2?FežÈò¥?B10+ᲊ?ï²cUԍ?"€ˆLøÔ?o«2½$_Ç?wÈ£¤2Åg?w(4þ™¿?|f9©œ¬?ï6`~	?…Q¡´û\É?‰HÖ-²@?yšÆ_¶L?'÷îÀÉÉ?zÐ{¤Æ?ï´1`}̽?yd]¾ÊE?22Èjr<?6{*9<Y?'bœ"s'?xȼ³•}?ïúØ!Ù]n?AC36I¿µ?9vC"Ž0?<Sq– Ô?0-|FZB]?-ð)¾7?ïãhé<Ä?f‡؛Ÿ?X"²}p?S"ߥýã?`îË´þ?a
‹XäË?ï'õÚP?sAeK™f…?zÎVT=v…?nÿ
¹wQ?|#. Ñl?`æ¦ãe1á?ïóÿ2Vƒ?Nû¥¶Å¢f?*kEë&ò>þ4Zïô¿P?W_Œ‹Û?N¨•?ÏêUAGN3FGL J1039.5+7324@`׆`ÔV@DG(àÉÙÓÀ:fK†ýÀ;éäwä=,¿÷æ©IåÒ,@ˆŸã	Ð
@À6 %#ü¿æ6…sO‹Œ¿ØŸ¹ÌÈx³¿á¤ºiÈƃ¿ãÍ
ñŸÿUNASNone?ïúÈÁ'õF?Hc鄡Ž}?*¥'¹€ƒ#?1	å9T?<g,iÌÕ?AÕÈ;W¨p?ï›Ývh<)?¢v+Éeä?rP þ¡l?'k@^͒?Á$>¢ùÒ?ŸÜ•
…ß?ï{÷͒¬?y§GÑ~£ü?{b¶ßGÊ)?o¾°yäÙB?ƒn&­uë?pã†é»à^?ïÑtË??A?oà–ûÓú)?0V
G1ŗ?2dݹ ±?v@9£´(}?o#t­à¦.?ïýÛÚJ¨Š?J)ÏÛåܛ?Ç)õÿS×?/™…Ê=tM?%ÞÃabÂw?BÜR¨­‰G?ïàÏÿdØ$?{R+<·õß?Z:lx$Z"?c¸¯lë>ì?bÊ&¼Æ?r™ÿS0vd?Xƒð?kôë`Ëñª?n•Ñ,v?aqû›ó`<?r *ÐÁÒ?c9"=¦Â?ïøm'Ã?F_† é?Ý፤B0?f‰ ¦;"?NY㈊§«?Ff­~äAGN3FGL J1040.5-5926c@qï™Ã‹«¿å¼^pÐÀ8À,ºs-õÀ:KŒÚw?ì/±>âúó@}Fößoè@U— E/_?ïÿÒ¯Kè¿çœ>˜ÍÔ¿è·ÚÙ8C¿édz"o!UNASNone5?ºf"§Rrq?Áš¡Ä4?α2»FÆ?̆ù³#?åîüD,?Ðý¦´_C?…¤ŽT‰?"f£—5v?ÌóË^©÷?Ã
^ y)?ènޖ4 ?Ãi}-cw?ÂSŒ¢˜ÏM?¨q«±!µ,?ÎGQ"-…0?±èÜ¥lg†?ãÙHrNjá?´]°‡1?ª(ê3SÙ5?¡»N4¡\?ÊÐçõ®T?¹~ÐAaÏ?çÖý#?¼E6Rwq?¢½(óÕÿ?¶©¸-Ü^?'nx¬(?Êçzîú?éqçà"B?ÎßË?Œz?Ÿ¨9˜È¦\?«¶?¨ÈœÎ?ЂR™ï™š?ÂÅÀÚâJt?æÁ"æ4/?ÄÞ!b?)%?ÎÌ`a)L?±¨Ïi¡ä?ʖßCášÿ?­rÁ»56?á§0-oNí?³ëùW­+–?µpä½$O?«kÆ÷›Ž"?Æã¶?®@o¶
,n?ç²"E¾êÑ?µìďS©ýOTHER3FGL J1043.6-5930@qõ¢£Y6¿áʇ㎰2À8'oJ:¶µÀ:ɵÁ?ï¬çÁ½¡@˜ü§…ëg@†ü L{¯?ïïð`OËð?Ø{W­C£!¿â¯G›¿àõ°Ý)UNASNone?–ð÷3ô?"¿¡ÍC?¤R*.\ƒ?¤
9Û<(?îXß?«AœÂ? c¹\kW?²ŽÀ¸òn?ÊÍ"¹yš?ČŸØß?èF{»üß©?ÆÚ©Eµ?ÃŬ/L?ª¶û,Æ,?´Lv²§? î~hß¿"?è…-'ç&H?°ÝH'@3?µU¸¦É/?°¬Pµ·øÎ?ÓªRWs?År‰¬?ãԉ¿±Ü1?dzTœ ›R?‡
¥xߊ¡?‹
`ž?˜Þ©´'ðè?Hgۃ	d?îÜàN®þ?¢*L+hØ?°
e^_¤?ºCÃ}‡"?ÍUðï¹-U?Âv&ýÍ?æ¨×å‹?Ƭ5ì?ʧï•'?­}bE3T°?¶^îœÝA?¡ÝˆOÓ?æŠ&Gp	±?°ýmæh?»¹Þ{©w;?³˜'%º'P?ʍ`חgK?¶LÀ–ì<À?ååkú¤÷F?Àë±>{æ«OTHER3FGL J1043.8-5851@qñDЩ*?Ÿ2±zƒKFÀ9qÁ
|À:¶,A§j=¿ãx×Ko®Ó@öôØ·›?þÒ_‡$!¿æÔ)9¬–n?ìS¤øûÝd¿éúvÚ¡X¿Þq'>|UNASNone?ÞÐ3±TÞ?ÌNÚä<«?­ƒfà<-?®9».1<?Ý_Šîʽ?ÌïDP/B?ܬ%S\ڈ?׿TØä!?°5õuŒ?´–÷¶?C?ßF™¯
'v?Öp
••?ã®"—@?·SvíV¶ï?¼EÖV–î!?§~'h¯Ôµ?ÒÃ-A+ÄT?´–è¢0åþ?åøÍâC?ƬAS©Â©?µ™Z©ÙS?ºm†Jô?ÍPÇ-Ú?Åbz˜qV?æ±Ã`ù{?ÊÁQGàM?˸J–?©ºNk¯Ø?ÐËØü0Á?ÉN²É?à˜')wa?Ù‰èîãÅ?®ûóaOë?°€3áB ?Úð`Ÿ@ç@?×"¬^‡?遥
@/?®££dœØ?°êJÆ~¨G?Ÿ€ïúZkà?Á†|¯Ä ?©LRl?êâVŸæ?¶4ŽÈ/Y4?‡'èócØ?ƒóðZÏ ?Ã&ú¯wì?µÝ?ˆöeMIXED3FGL J1045.3-6414@rIº^5À–§}‡ëÀ99ÀgmÍÀ;ú¶êã8?ôœÙ!™Ø¯@Ép륀@êvà1-Ÿ?î…а噿è5q—Ù[¿é°9é'BÜ¿í ¯"VU;UNASNone?Â0‡"*ç,?¿tœMí¸?Ùèb('ïÎ?Í{òE=ˆ?ÜÿZz}[?ОôËa?µ/ð'ô'?ÀðÔz&?Û5ÿÒÕó?Å[9½øî?ß~éÿQs)?ƫ̒üW»?ÔRÁÿû^—?²°øY8C?Ø¥,û
͹?³Yš¥› &?ÓùÓ°?³u)výÖ?Á"—ëªÄ ?«PP`¦Å?áu4
^ôh?ÁZW¼và©?ԄKïl´ß?¾|"š7_?Æ)ÈT±ÌÛ?À"®(¥nB?ßñ‡L"2?Í`ºW ŕ?Ôù"‰—÷a?Ïv‹³¹?Ç
´Ë›–Á?ÉÜE+¿\³?ÚænԞþ2?Âó^9¤Äù?ْ¶Å"6m?Å
µ.å?àhès"Ââ?³YÀ´?Ôaä«)¨µ?°À«Iwöº?ؔ݃dŠ?¨1ÜÈô?Ó6q3Òs?°‡º£CUY?Þ$t­À±Ð?·ç4õ-¨«?͐©Â÷z?²A1×8MIXED3FGL J1045.5-2335@pуùd@>à¼8*ùÀ:gK-û»ÎÀ;Æ¥®zÒ.¿ÑOƒ@r@
ö"»Á¸@ð¹@}ôx¿á»`…É$™¿ä½'J®¶¿çÈóœDnÅ¿åäS'¢FUNASNone?ï³±1Þí?}
Á2?fæf`o?dsÏ-@Õ.?z´3ýÌ1¼?x+n	Fk?ïT2ä¦)Â?™öÓ|+"?'Ðíý
M?‡¡W›JÞE?ˆ#&ށ¤1?"µˆ@3g?íÃ÷µu?™:/úå&?™âÛÐø?ˆ5ý•?¦ù5¤‹7?'½f<í¯?îq'z¨?–K0à/›?Œ "žWïU?€x³ýìR?§–ƒûÒ½µ?"Ör[õƬ?ïéaûȍÎ?‡°±꫎?L…ú;&x?rßФ¹ƒ}?^ù9»+En?}Lf ´z?ïÊÁ˜!†?z–šB'LÉ?h3zûÑ¡Ž?f¿.àx[?m®Ã92¡?t?©w(ô ?ï,d)Ç?†¿-`?†aú€k¦?x'}Þçÿ?Ž"û9ãÊ?õ­WG?ï˜åÚdåÞ?s·Ñþ8úM?l±›füJ?UŸÂØ¡$$?'š"Œç~?q›ØÕ@ÿAGN3FGL J1047.8-3737@qW8›R~@3Á;ŸÀ:#`m(!‡À;­ÓÞ9Û¿ÖܙAÃ;@¸
n˜å?þR}`}ï?»ÀÝf‰2¿Úœ91$T¿Ë¬šlu¿çi øÈÿ
UNASNone?ïõì0?O,UäËy?BY©äE\|?CîÆTŠ1L?Gf¤é¹?Ae鈤\ï?ï@'ü"†ž?™¾m0¢%?€(W³€U'?}ªœd¼Ð{?Í©4¤ôØ?–%R¥n±?ï5dM²em?"qS/ú?†ÉÏ[6KZ?{•§ÈŒ›?‹ÝB-<?vÐ̲PZ?î¢8¶Í(Š?"%0 Å?qê®RÄä?mø™C#?£Ÿʸ£à?"Ü7d?ïû;G[?5JMC`?*°A¹µá½?(o™ûõ?49ë&B[??+lÚÓÃ.?ïÁií¸v?›ç³ü?g+ÄçÁ"à?_a™ò]Á®?sµ&ž='î?zdSõG*¼?ï•ÔAz¥?qQe:%›?yÞ·õ8S?kҕ
T?{7()¤?`1Ù­åÖ?免BKý?q'ؘ$R?`V¢êtTE?PÚE?½Æ½Ź?p0ŴՊAGN3FGL J1048.8-5006@qºQc4'¿@ <½ý&À9ýýQÏÖmÀ;pŽÉ[ÿ¿ÖyÐä½@
@¶
Í@cƒ 3Ï¿ëhÝûÚh¿Ó4IèE=¿ã2>^4"°¿êÏYVTíºUNASNone?ç³Uh£h·?ÈA;ÇßÛ¦?Ì…
9?Ņ_ÆA·?¤`•$ÁŠ·?¨7›0W?ë¤-Êú ×?Áf°Ó?ŸÅ%œCXt?¡È-S:Þ¥?ºíHBcý«?¾‡qÔØ?é¸L­á,ß?­F¬+ªnL?½ÌÜôÚ_?¥ïðõ=\Á?´p½Óç©?Ÿ£-â©gt?ëhÛ/ø&?¥ìOÕƒ†?¢IYÚÁx?"Je5@V?»šÄ7¹?£½`s2Q·?êзøvÁ?ÇÖN*ÛJê?ÁÌ"'ê›?ĪÜU¥›?—‡ì^g³P?£è óù3?îÐdþ®¯?§·oFΊV?"4[l,aÿ?‰j|½e³?›Ù2t™6?¢ÌÙ)ó?íD߈ï°Û? 9AJe8p?¬nÝ·¹fÕ?›0šOí–+?ž†Sw¾€î?V"P«ÌÊ?î"
ð¸©?ˆøجD*?†%"•ý
‹?sǡݒo<?¡5ìA®Õ?…âWØ¢ýAGN3FGL J1049.7+1548@luâlv@MÎ#žj¹²À:Ë*5]°À;Ò·£oÜ1?¹'ÄD©Wq@DÄyl'›@9Qx Ñ¿ÇD£¼ãýV2ø¶ò¿Ùô"U~{u¿íCWŒšUNASNone?ï±M#£?ƒ6@ó¥~?€'4‰Kw?ÿ	A–…?XÔMêx•?T‹+Ê5§-?îò#4Ð?˜ÂœÏ{?'Î/"8?ÆЇ&?ÛšGŠ?Ž÷[ˆp?ì_´Æ?¥ýÊGk·O?·?KF/?¢¹ÍKåÁ? Óæ¾ÝÃ7?Ùk/ôÈ?ííû,6?ž&Uü½ó?›¦Î,ë"?'k¾§á?£WûänRd?•d¾€	ÎÖ?ï¸V.qÎ?*0dP©?~©‡©|B ?}ÑÓÖÜ1?T­"sú?O1ÚÀ×bò?ï®Æ\EPA?zjƼ¢;3?vÛjQ?p~Èáœo?rÐÛJE?pÕMoÝ?ìþßßN.·?¢¶«#×?²L¤»!-ì?ž›†k™?–ñq-%
g?Œžã—R?ï|…#ë†?yH~Š¦·ç?ÂyøƧ?míݧ/@J?~8{Øü£…?rd:#Ö¶"AGN3FGL J1050.4+0435@n±
gb@J´Ø]ú‡À8ê'"ÂÀÀ;s˜~§?ð%²úh¼W@ªð†y@ÂÆ ‹:Ü¿äæ}MŜ¿åmÏ557¿é¾Š¥ñþ¿èéM¯VUNASNone?ïú]āNÊ?=gPõŒ(e?<(\0l½?5à!E¼Ä?0él?*·û¾}?ﻖˆ[ó`?'õô.׬?nð÷ʊ{ç?y¬Á¶6'ñ?r¼?ߢN?v¨¢³?ï3³ßýt?ƒ ¤čæ?‡éî«Ò#?y˃¬1s®?‹)N¼˜Ñ?v†E_HÐ?ïÕßÃI–L?vèµô¶¦;?S{¤K9?Yöt'þj?pLQG\?uR"ðÀ ‡?ïü±Ö@,Û?0ŽQ,÷Ñ?2"Õ型i?)ýåP> ?±Ük÷žn?h€?ˆ™ò?ïæV"mà{?f'«°öÂ?W+·Ç_®?T¿.…wÄJ?\(p,Š?_¼€'Ï2}?ß^þF?qõ"x'Æð?|¤ßð®dë?fƒÈÝeŠ?|"°hˆ%?dåi
	‹?ï÷Ô÷­dì?Rݑ.¨ÂQ?:Ëj.©ª?7ÔÒ­`¡?CFkϖK
?P‡
b'ëAGN3FGL J1050.6-6112@r {5*"¿ú¹ýl§ÉÀ9gâTÀ:"Ö)làÔ?ñ^¦ß'mW@
á>µ[E@Ñ.à=B?ïþò7Y¿ëç…* åÔ¿ïÿí›ði?ïþ¾M¥UNASNone?½·5¿]+?Çõa"|#4?¸Š±õ0?ÁÑ™»(?éK÷ÃN&‡?ÍèoÄ;©?É	^¬r?Ðú`'¼Ü?±Þ>ËÀþÐ?µ5 ²eãø?ç}µÎêšy?Ñæ±ò£C?Î	u£ßÝe?´[W(x?Ëñ#{&´A?°Mñô
S\?áY¸>[—?·¡û_SÅ?àËäE "V?ѝêz?¡ë»Ovà²?ºesšº?Ü*À
Ð>?ÑŸzje‹?¸
HiB'5?Ç©}Îs&?´Þ>ÞéÙ?¾czÓA?êb‡
î?ÉÈY‹·C?×9Ì5Ç?×7õ0)y²?±Ñðûý¨<?±¯Âꏚ+?â(ÛÖLtÅ?Տëjíp?à'Xksbñ?µÐÒé¤ýY?Ãò
˜y!ï?¨'yÙm–?Õ¸IÜÜ©(?´ÉÂeYØ?éOž.Ã|?Ãü—†4Y?‰s™†¢'¨?£®Ø¿ ?É,»ïH¼v?þþFÜ!BMIXED3FGL J1051.0+5332@cUŁo@KÁÆ*\}À:{ˆe"¯OÀ<ñ¨Nh¿Î%+Ž@™ÿ¯Î@﹞¿ëvTÀ*æ¿áº—âÏ}¿ïÿ)Î'V¿ÜZN>–,–UNASNone?ï÷Cicº?U{¸—:‹™?K°³y'¤?S?¿ zhŽ?-–I\¨`?6™FJ"@Ø?ï•U'k?'šˆJõnB?yÏKý6{'?ˆ/ >"ßL?{ª‰J¨Úÿ?ƒ¶[PCžj?îP
}'YF?—bžÛ¢Ó?˜c+ªò,?äÑÍÓã?›$ϑNý?e~®š?ïÛw8Å?"¦"Ó¶î?ˆ¹\8­I?‹ºˆíóå ?ÇãbBÐ?‹Ùˆº&Á†?ïüæÄUì??Ê¥^KÃy?/k.Bv?8Ɉ+èÅ?"(º<8?( 9àßg?ïݯžÐ?t$€æ¸çÙ?`PQ¦¹±H?fçnÃTn?bQtýY?f›@ôì?ï2Nâ™ÆC?‰Gá¯Ì¥¤?‡nN?Š¨OÀã°?‹ýXàW?'E
{ü÷?ïãã8ìR?fWÖ>²5¦?Sõ¢âÎ*î?K««¢xc?b!õ˂¯?b¯éÓÊîAGN3FGL J1052.0+0816@n!ßzNz·@Lr)ZlÀ:{¨G²F9À;ã!"Î~~¿¦FéC\~@Í\%DÞ@ÉÇÿÞr¿ØçJÿz'¿è¤¢P¿åGrI7p¿´ÃÂV	¡UNASNone?ïÓ")è?r.šÔÎj.?Y؂
e(?b@䫐?oû*š"­²?jïKP?ï£óÔgd­?Œ™r~ãåâ?u¼þFÄÿ?'¨áþ:™?xIš'=o?…«ÓŠÜ?íïÉîîW.?˜1Q|a‰å?›"þFgN‹?\["~¼?£qáí
þã?Ž0×âuB²?ï…ò%t?'·N±'?nê¶eââ?wŽ>É ¼³?™Ñê÷bÖ?'{–`)?ïòT▞Ï?W҆èïo?AP›ŸÒ?HŸùB¯•?R­òêŠLF?P9£…ûØ?ïàž2Ût…?p†´´6ê?]–è ^»?bã]ˆ eÏ?`–YOÔâò?cXç¿@Ãý?ï,.[ªm?ƒó¡€Î[•?‰F²F,ÂÓ?}œçCPû±?‹­¶Ù†É§?t'5"ñL?ïÛ"÷Hv?i•eìé®Í?O¢éêV?OЄ«Û¼¨?lþ°°È›v?f˜|€ÂAGN3FGL J1054.2-3123@q7KƧïž@9'¹¾ÓÀ9ëUmßÀ;³'ìüíý?ëçBXÑ9@h|	泩@ÀÚñŒö¿ãFBÂGbÀ¿ëSVÞÖ\¿ç҆²X¤©¿ïþçSá©~UNASNone?ïžáêÁ)?¡›Rô,?t«ÙÄUë?thrŸv?{ã0ܬÁÒ?¡[fÞjÖ?ëÙÒq|o?³ïà;(Dú?µ""N‡ö¥?¨2€ïtY©?¨°Ot¤›?­66X7Á¼?í¦Ï&??¤‡:ÓWÙÅ?¬zÎ%³?œXEƛ Ô?£v>ò?'6ÜÑuÕ¤?æÿÊ#‹[¤?±h;û@?ÈG­NéXZ?­MY1ê?·rTDˆ—ª?¥ÚSj'¢)?ïmŒÇ'êî?¹6¹šÀá?rMTû®Ã?‡ ÈJ~v?‹v#¢æW4?¸í¨çŃ?î\µ2ÚÑP?ŸÊ
ƒÍ? "ë'(?"jµXükW?"_ƒs<¥?•ybCK?ìR?'n^D"^À?œ3F= þÅ?‰ßN©Þ¸?«S€Z®L?ƒ›­Ôe?ì¬(>&p?—+B¯_Ñ?´ÿ'/¸—p?'H$Ø{?–|¯~lÜ?‰ÓS®æ£\AGN3FGL J1054.7-6006@r
£Âˆ¿Ý'l¡"ãøÀ8…æ<à[À:7 Wù¼?æ¿M:ö@
Æ`Â7{@i³ +9?ï÷‡'að>¿êò1¡°¿å±ÊsbοáÉZ
§<´UNASNone?ƒ<¾*ùK?‡‰ž:?ƒxŽ×}¼?Œ0z÷6®?ïf¡¢Ûl?•¦FŒg"?¦ òv"É?°Æú=ïî?º¥q>0½7?¸VÖ)܌!?ëAPx¤'­?Àmyå
$E?¹¾rl3?ª'}Š~Ð?ÁšñóÍ–?¬Ê^}K˪?æêÓæúþí?³ËEÒâ?Áia/<P
?´=ìXZ…?§Õ؆‹Â8?¢"e¯à—€?ê(J+È/Ú?·œÅ¬0ÅÒ?'—×Nè?‡F§"Q
J?u—w"œÈ-?}žÑÍI¿?ïŠt¢‹¨?¢ìúJÒ?¼¦w3ÏK"?Ù@Á™Æn?ÀЁNìn ?·û`‹'ˆR?è7ÅÊúæ?Èå:(uâ?Ï&`4"R?±àS®§–?Á–5×'n¯?ª´Òá?ãÐì2)@?´¸­tܐ?ˊ§y‰·?¹+À®HŒ¾?®]†gêsG?œW_
]™?ç7¡/BÁN?»&EW*¼ËOTHER3FGL J1057.6-4051@qŒ¨$x@1ÙUmÀ:yߙX+:À;Äîð
Cµ?äQSzW#@
êÖxF?ü#Ÿ—_ƒ¿ç	­³ø¿âkrÐé"T¿¿}t$¿þ¿ÁÁZà˜¨ûUNASNone?ïóÔñ^|?OôˆŸ-(?4'`V(ï?/峂‰Áº?SS$ÙSó?L–oqq?ï"wé4?'@ú:&%?sž`yL¨?yò
¬à?…Õ{º9?Œ—7[åBµ?ïçëa7}?"CJÓCüˆ?"ð'ü¢'?rÒ-Ä:U\?"ŠÁ?•J?~«n«Ëʕ?îý"}!=?".›÷uÙ?hZޟ:së?{‡h-®Ñ?B48RÑ?''Û	œ#?ïú!Â{×?=Å·.Z±.?'¥¶¯ëDÑ? ëKÍÎY?AˆʍF?:ƒÖýá?ïÖÓµ/ˆj?t#ÛÎ.¹?]0ì~×?VÐAýu"?j"<ð¶M?q4Ìa¬;2?ïå.(Ã?s1á˜Æ"Ø?xI§~Š¥°?b`_é+œ?ƒaàÁàƒc?m¿TÔę?ïÁ½:D?s	Öb[˜?e"lÝ e?fªfEÜ9œ?tëG-b?jv¦r>žAGN3FGL J1057.7-6624@r>1[W>«À}'ÔÀ9«'!üÀ;<©Ôz@?Éþ"7ëÝ<@.®oês§@­-êñÑ¿ãG=Çå:¿êÌj¯ÔÌÿ¿Ö—¿s5W¿âÛמ%ß'UNASNone?é¸ËU©TÎ?ăïÕ ¿y?†ó©k¯ã?ŠÎۗVM‰?Ç»Ãm±
?Ärée£Œ¦?ä†dlÍ?ÐIžÛ‰m?·¨­ù®õO?¶tÚµ®0?ÑêÈ]ß±?Ê"Ï$Jx?èÌÛâƒ1<?®'ꪍš£?¯"u7h
Ñ?›.ÚD?Ü?Äës&Ï]Ý?ªgžÏØR¹?àBC
ä?½æŠŸ<?¤Ýµ¿? lÂWF'?ÜßÁ"€g?¾¤|:|íU?ëð®{¨î?Áae¯¡º?†›+=E†?'´µj4Æ?½¬™Ä•Nd?ÀʶDþ•O?ëhPmœ?Âޕ—VsT?¤ŠY¹ôqÆ?¨–8KûÇ?ºxRü@¾?»ÆϘë/?í7ñD6¡ä?ž^ëð>ñ÷?Ÿ?"'—–?nþ Nô?¬ºL*p®ù?—WÃ)m´$?èÉuŒ?±¢*'ÉÈk?£jˆƒ‹"?Žv˜ï—Ö`?Ë ê¹ÐNj?°ßa6,¬AGN3FGL J1058.5-6106c@rœwškQ¿ò¨´wkÀ9&5îþÀ:HDK‰kN?ô—–"×h@E¬5¨ƒl@BÁf½y¿çZÙÀ¿ëûÑD¿ÝAåu´œ¿â_¥&À‰UNASNone0?'êÂ5'|?'\ÝÛм??€"Ri?Óèø'Ó?ïsØÞd5?œú°I"9}?Ãb‰Þ¡Ç¢?ȘÎò°¥é?½A\Ûg<?¸½Mà<þÿ?ç1ìê­?ËDœá'nÂ?Æßð\Hö?«z0¿,ԉ?À:ØI"Ø÷?§ÄÒíÇ[?æ9M×#gä?±ÌH?ðí?ўÄwyðB?ÅcìÄÜ5?¤Ñ+Õf'i?«]ÛC\|?åã‹Ñ!è?Æz-5¡?x'D´ˆ?"/k–?€#œ'?—Ù8npü?ï"'i8B?£°>t8I?Ðé8¾7ˆ­?ÑÖm4‹Î?¾4¬]&Þ?µ×ìÀ§h?ãÄâ‹X–Î?Ði4Xï|Ç?ÑöMŸE*,?²ª'Hۍ?ÀÄNÙ¬Ú?§x~rÊîh?âÓÅyò4e?´ºÔûx?֔ƒy`'æ?Ã>©|ï?¾wqY<9ö?±d
‡ì"ª?àæÐ(7N?Ä8¼»måóOTHER3FGL J1059.3+0224@oY4Â@Jį¢ðZqÀ9˜ô¯úÀ;L"ø?Ûh_¤D1L@ªæÂAX@ÐßÀ‹¿´1]¥Í"ƒ¿ä¬ùAc¼W¿æÂ!=ƒ`¿é§"ü»kÀUNASNone?ï	<Íè«?ŸÑÅì)ƒ?œ3!üw?Ÿ'µ¦tÜ;?e**Ãôq7?`@1ͼd?îëhQß,? ääC&"k?':þïäÈÐ?–Js¾) )?WöÔ5¶k?–©6*ðÁ?ìÒd©?¤#|R~*'?°ƒ&Ì®«? ¥wltÒ£?¡¾¸ÔñÆ?Ž-½Yf?çë˜:& ?­hz'?ºç>¤;Å9?¤Dø—%×ó?ÂÝÿÃ!ÛÐ?ªò?0…"õÚ?•å½Af?|m¼%ë?€éwU1—Ë?U(y
?ŠÇâååbö?ï,</Ar?Œ^"oø~?zn§«:¸Ü?ƒ3Ó¤$à|?vû:7¥.?²€ˆ8?%£õà?'™ýL5?›øW:¥Û?Î¿×v?ŠbÈ"ù<2?{‹™¡0L³?í34šçL€?">¢‰¦?¥ÀÁ:mEE?ˆ°Î-cÕ?§õò½?ñµß'AGN3FGL J1100.2-2044@pë•a'@A‰°¢ÊšÃÀ:H–ÂNĉÀ;Öu¼D¿M¿ï-Y[ÇO@þ\¿sÜ@MÅ¿g^‰¿íF½K¿É€tR8S¿ëA¤4Óp¿ÜdÌFÚUNASNone?ïÚä$#Ã?xà(âàÕ?qžDqm?w¦ºܸÀ?6&ú®;CD?4§±Á'ET?ïŸÛßܖf?ŠÎR³?sô†.=º%?|w•;§¨%?|‰ÝGÆú?ƒ$•&;½?î^ž#/—?•X áÿ'\?›;©P%?'«œŒ¤O?–ª \iRù?'ÁÖo§ôv?êCÞ°?öܙŠ1r?d:C
i÷ ?gá¡àÚ߬?‡Átµüª?€jŠ§';?ïõGF?^èø" F^?RZòÇ_³ð?]Þ+²Å?(·¹Ÿ?ÿ¼?$'_ÒÇ7`?ïßhÈbÒ*?j}êøðí?[Îÿ×^_?V(Ü
#Æ?b¯¸
d/D?d`_"&˜)?ïDÓGÿâ¾?"±Ú-?‹8¼V_ÿ?€êÒ8Æ?ƒ'q°g("?p(éøfŒ‡?ïí¹"¬g?Z-üô"W?0EèÒ®t?'O¾‹kÛ}?`Fs•·?YWˆÅ9o2AGN3FGL J1101.3-6032@r²-V¿àS.øî¿À94íbnŠ!À:lÞÁÁÖпÓØe—^€ê@
°Øù‡Á?ÿu˾Úƶ?ïá…ï¡@¶¿éᖸ52‰¿âV?Zf†¿ça
˜¥UNASNone?À"§cd\?ÁYÌ,Çg?zŽÒ™e¥?|ìIŸÈ;$?ë¦'ØŠE?Ás5ú_Ø?¹¿9ëw÷w?øP5nï?±þŽÒˆ{ú?¬êúÙç?êˆFèi,â?ů!k4¬Z?ÔNµ`°«?¸I‡ÈÊ?´\"»wØ?¡¤™~\K?ãM ø2–?¹<æIÒZK?Õ"¶:††?Øõ€†^e?††R?€Çҭ݁z?åaØÚn˜?ÃÂÝ?‹±$?Õà?f®pý?Ο.Üü	?'Ôöm)V?ƒ¹‰¥c?äÇ°øÓ2d?Ѝôʱ?ͺ¼QÝöÉ?ÑeuƒBs?µ´Åt1ãÏ?§Ñ2[H°?åÚ¸=´?ÐÙ^}}ž?â4©{ £?»]I‹~Ã?°¶é<n?'Pߓ?×i&
Ÿ"Ÿ?ºièňS?Þ$µ­‡žV?Á:¬ˆM…´?"ÜЙ?umò˜Ù–7?àš1æÆ·Ï?Á4Ý{àdôMIXED3FGL J1103.3+5239@c93Úøßz@LÀ!ÀD(NÀ:At™/À<¼²£V¿¿iòC÷%@µMBs@ñç_u0"¿à"°¦Ùý¿ê-	ﻐ¿åSÅÀÐ%ƒ¿ïþ'ÝQn!UNASNone?ïÑx½ë'?°ÅgÁ+ð#?ur«þÔçb?°ÇXiS?=U´8ã¹?;B¤ƒm3e?ïxùÕ³??–r¬²à?\Œ6ÉY•?Œ¾K ³?ŠÅ5d÷â‹?‹]âK×?îíú¬Û?‹â'¬¦–Ì?"'Ö›qyÚ?†RNYy?]Í뤷?~ÂGT4+?îZãœ6µ?œ'Ö	vF?›ÎÉuV"´?'`ùr¥Âz?˜ÔÓqûœ£?'ýªd7ø?ïǂ#EÕ?³W+'Ù?{H+ƒÃ½?³žyBÛ¨?.Ú~("; ?:û-.ZA¸?ï¾Á` ëÍ?v2ȒË7?q#~ÏÊ?j(ñd~~9?o.XÖwoÊ?mµðWåq?ïPLÙ?c¬k!N?‹ç´d-Å?~4faMjÉ?€D£Îâ?mí‹ëzq¿?ï»}Ww=Ø?sÖÀ·?rü©ïµ''?cpo»çÅ?n‰TÏÓx÷?lØ°¶ŽÃbAGN3FGL J1104.3-7736c@r'—CécÜÀ/é‰XÙµéÀ9ul¡
ŸÀ;Qý¢W®=?ïd»þ8@O¥ 
Œv@_y5¿Ôpͼ¥§¿éM­TXê¿å_Xœ"ü¿ïÿGã<¦UNASNone!?îVË¢Å??¦™ª
ªþÇ?£Rº{Ö)?¤\¯ßO]?ŽKÌdЗ»?‰bI«'•À?à\8y‡ð?Çd®f7ö?Ò«+"©´?À—í1œ/K?Ê}ÇÁu*Ï?ÁŒµ¯P?çô˓Ö?±4žó¬§Â?ǔèòi¶Ê?«ªà]¶/ ?¸F«Ú¶?  ¡Á‡ÿ?Ù?'æFñV?­]Yðª#?ÔUj^ÝIá?±¯"V'é?Òk¹Èä
?¬P"%3Ù?ïŠÕþÇ?˜v_R¬è?"nbor?•XKt\ò?€S€˜H?y9þq,Þ?çngè$I¿?Á¦'d?ÃíðŸP?³úC[•3?¼°à»Ÿ±i?¶J²×V‰?êþê.ç?§¯º§¸£?¼ÂpIálä?£U~ZАd?¦Œ|'`Á?'[:ܖû?äqò‰8½?¢˜ü3ïP?͂å'Ñ++?¢@´c?À¸²µ/³]?šf4á_á$AGN3FGL J1105.7+4427@dÕô!-w@OSS&ÂÀ:Ž=EíÀ<;tÈ)¿³"š²@
Îò+Öó@>Û_· –¿ã[ºæÆH¿æqrð§6T¿ä,OÖÏQ"¿à}J$þUNASNone?ï®טœˆ?‹­ø4Ǘ?zfmŸL*?ˆ×08­?m¸[ß?nÕ"Ÿzκ?ï…ä"ª?¦6¿"0ø;?@lJ¹´-?Ÿ|¨äçÖ?Š®zqù&?"¾>0ë™ç?í½¾çÜȘ?—Yš…dÉÒ?›ý±jG{Ò?Œ‹®PZÂ?¦%8ÐTŒ?¤Æ õ¾À?íLi³€~?¦<òûdÙ¬?£ê"EYw? wTiF'!?§Nà'Ÿ´?›Ë%Š¼ú?ïñj[½Ê?ZQf%Ùv?Hoþýr€?Oÿ›p•¡þ?PëDõ»øü?PM.Š²…?ïÇBÁ=?'º|® h ?m*°ÃWß4?wôh˜"?k"2KP'5?rNhQwh?ï-m¬*ë¼?/ìc4gš?†ô𓌠s?wì"%t*?¯¤e(‰?tÊMõ`ÿœ?ï'-‰Ðù­?ñRF(˜L?>¿ð¦´Ë?r[V¶x?|k»0sÞ?súXxH…eAGN3FGL J1106.6-1744@pçquŽ!–@C7-À:BHû"±À;¿~6fÄZ?õòs´@
2"a¤
@Bÿ¢7"?îmÇÆJ)¿Ð÷–±Õ¿ádZäªm¿ïäÈQ'ÃUNASNone?ÐöÚlȀ7?Çùé†?æ±@R318?ÈìKkõX?šjNîÉ£'?—P'¿à?´~J@ž‰?Àï+ëÚóÆ?êÁítHc?ÈF<Ëôpç?µxùJùa?ºÓ0ØÔ±·?ÒîÂf¨'À?¶D ò7L?ã'œ-6ˆÂ?¹,$"]Œ?»û©rï?¥Žæ•ÔEÆ?ÂK2× kc?³-¨ù–¬?é@ŒÚeß?¸¯r"Š°?¬ÿ+Õ×ô"?¥7[¾›s?ӏ¨˜Ô¼?Ê`Ο¾Tm?åÂäOS?Êüÿ".0?–s(â9€?"áðµ:??…´Ñ>²©?Ç0AÜnUs?è­âlNæK?˞ùþ'Ét?µ…'üÃ6U?³‡Yh£˜Ñ?à	´¶Dc÷?³•«,Ñà¬?ÚÚ_ËV:?³ýq~t/?´HÛ ¬â?žŸÆH=_?՝Èøן?´å,zÖa«?ä'ŸŠä
ö?¶.>!<á? —¿"!Ó³?—_ˆõ´+ÿMIXED3FGL J1112.1+0500@orÓEŒÒ@LÎéd8À:T…òó¨À;À°',ãŽÀç§íå@:jôºL@¾ó ¡Ë?êÿßfWwá¿âóq@"õ¿èj~‹¿ÍRU`7UàUNASNone?ïçۚ߮–?cDή©Â ?T1r8´t?SZº	tµ?\Xš Z?[SÎÍB¿s?ïÃ&.ם¥?¥-µ¦÷?jâŸÛq½?x@^þQÚ?pû˜‰Rü?t6|鵐Æ?îP@5éàž?–I[yß{6?—ÝOz1a†?‹¼ùOt¢ã?ž©Á³RÎ?ŒRjõ±j?ï˨¤0]?€¶ PiQ?«˜Ø3þH?:.œÖ™?z§eDå?€¯õ)xük?ïô2®lÔ?T¡ŒpPöï?AïdóJzµ?B:ä}þ"…?MÿЙ`šš?O(£Î'†?ïé‹–\ß?fT´:æ†?TO÷§Õf5?S€Ð(°¦?Y¤ðÿuÛ=?`Ôª¦W#?ï(Ã<͈+?ˆe´ß*?Š¶²'ߧJ?€bî›ÙVÊ?‹~E
!è?€ÙÌe'?ïøfDÇI?Q…ô½«îm>´m[·5Ò>Æ~Ý'?N\µD¬°þ?Q"q|4§ÿAGN3FGL J1112.1+1034@noY_í¦a@N¯hð"aúÀ:TËf›@À;Ë
Yö›¿´® HC@
ÙùXqQ@á'À8iÔ¿åK/99‰¿ì}0ÂÀ"j¿éÊãÙâ<©?áb$•ê;UNASNone?ï×U«œë"?r:Ø¸ÃÌ?GÛÝxØÂ?EÞR•/Ñ?qtn¨†qÌ?q °-À'°?ïºaqZ°?"†[«Ɍ?pêåç#?|'÷P!_?r³\-à?vˆ~Ö(!þ?íé²ø žÂ?–m½Îºà?•‡Ù±?[=?"tm•¥³I?¦ ã¢Â±B?'b̈AH?ï¦k¯P?†È,ÿèX?EMÒî(ÈS?_»¾ïSßJ?…7	ö[¹?†Kð½n•G?ïñ3qÇ?[µ"lNGå?2""üßúË?1ŠÅrÆ2?X Þytïl?Y›¿µÌM÷?ïå&÷Kâ"?l‡Cëç%?Y?½°Ô6Œ?`›ÀÊdÚw?\rSCóĎ?`ÁìZPÂ?ï(³I¡'?ƒoŠ²ºµ?ƒþÓfm«?síIÏîɄ?î€
XFß?~ôw( H?ïözâŽ÷?X•ñïö
q?1LˆüÙ÷?1'ùª2c?QW%ô5è^?W%ƒ3JAGN3FGL J1113.1-4515@qÕ¢£Y6@,z2	g‡ÏÀ:)ÆäUŽÀ;†N']‹?Í
Gö'¨Õ@
§ÍÓËD@–«ß—TÆ¿è2Ùhˆ÷Ø¿âÏnhF¿äT®€¨Ô¿å7&@l½ÕUNASNone?ï,k+gÉ? ,9¶-n»?zÐ,bÎi?€‡Á»XԀ?"¾ƒ¥^;?·ŠÉ±µ?î?zKß?±?ÀÀÕÌ?'Yà‰&¶¡?™"ñgN?¢Ûfä'ÁÂ?ªÁkgÿ"	?íx™_É$ˆ?'Ýgϝ?œü‹œÐ?‰/¢p\þA?ªtæ—…?–âO£Ú¥?ëBrñ³–?¤ÌµØlýª?¡Kcd/S?"?)KÏ?½Fßɏç¥?¡i<0DÝ?ï×K¸²…ñ?—Ø8E(ē?Qs›÷ûvD?[ÔóAí"?oúyfû¯?—{î{ÚÊ?ïƒ-io°<?"²5'vF?uF_Í}qO?xÿ–¸˜?"'u³¶P_?Ži¬\÷?ï-Úèõð?'Òöv°0Ã?…¹˜á½ê?t§—…VX?ŽÐqiq*1?zÛÿd¸ˆ?î‡Í.Ïÿ»?†×ù€Óݵ?òø 0δ?u•›¼kL?ŸÞxS?½¾Á¹ÍAGN3FGL J1115.0-0701@p'Â;yRÒ@HQt>–=ÅÀ9²!gXÔ­À;¥¥
æãÏÀóEâ¸Fƒ@ÛÄÞ@è~@ÞR 3Q;¿â¥ç*úˆ%¿äʑ5òÖ!¿ÛH´ª>†¿â§¡²AÜUNASNone?ïþt	g1è?l'‹Áׁ>üü¿]	×>ôíͬ?%éÃãpQ?ßÖE»®?ï¾éYlÐ/?…à^˜?n0}Y¶?/ÐŽVý?q»ۘ?u3¸œÇª?µÙ7·?t`
uš<?qíá¸>?_®Üó	D?'ŸÉøɸ@?pŒ˜
â?ïîenâO?a¿=O>܁SFúþ>ñŒr¤¢ˆ?aŒQ"'™÷?a-,R.?ïÿKÑ9Ä?àþ'U>ÿz{?%Pp>ö
Ɋ?ê¸_µr?
§[Gƒ?ïçÀ€Z¥µ?o³CZú?VºçsÌhi?g¬–ðs¥?YĢܯ?_Ž]\ƺ?ïÈ©i<Ñå?b˜l{†è?e,‡ܒL?KdÀÖ=ɘ?q³,"š?^¯hí½˜?ïýu*µœ?7í£ð²Î>¨¤ä(Ó0p>—o&R?7°ÌnNí?7êôèyPAGN3FGL J1116.7-4854@qõ>"åÞ@&)÷LsÀ9ÑûÊçÀ;veŒKÓ=?壪¬2ð»@—k0O©@­J 4¨Ô¿ã°ÝŒ§\•¿ç·ó…âòB¿ê&µ×›e¿á³
¶w½UNASNone?ïäˆðvl?dô×ëªV­?\‡S´›<?]1y9DÌ»?ZfËӝ?WtmãLÞÝ?î`}ÞtŒf?±	àçQ?‰£šŒm=?'ÛÀà¤RØ?£A¶_¡F?¬iûV¯?îŠ5¨zÕ?"¶ø5l"Ÿ?Ž5ÍãPÔ?¨<ë/ó¿?Ÿ¡ò¸×'ó?´ªÿãôˆ?ì–/¤)âÊ?£;s7sùf?™"
Œ¦.7?"–ø¹ìt?´é¿}­ ? §¦4£ö?ïõ¿2Á"€?R†ÃƒU?CT°áZ'k?CGŽ¼¨
—?E®ƒÉi9+?Fª$8pÌ?ï~í(ëdE?"×3qá2¤?s˜Ê?|‹âRQË?†¼éz¹vÝ?+ÿQBË?ï{þS¶+?zI9ï_ÕÆ?{5ªl\Â÷?n•Ú[0H?ƒe•ÍÞw÷?qDNÎ+£?ï%ç	(?…A ~þW?†¦ë¶?uY"8Œ/?'º¥¶f«?½†p«dAGN3FGL J1117.2-5338@r,\ý
@¸èBt×À9_Çȁ
²À;aHZ⤥?ϟNéÆO@Ô>¢ýñ]@uÿ‹í¿å2. ­R<¿Ü<
"¦¿ÓÒ×CÚ['¿â]֘[3¶UNASNone?ïó¨ÀÛ'?R",k£ÿ?8ȅ÷‰?5†OH3‹ñ?R}£xÑ\-?P&¦—"—?í ¨¹i	?´bÛÃû?…bc®mi¥?'äɌ´?°NmÀ/­?²Îƒþâ$¡?îü¦_[?Š÷UXïQÔ?†^³Gå?zê¨ÀÓ?•7"߇?…,ÖýÇ#g?î™B	‰g?',¾"G"a?jg4¯ñˆ?e~òJöùe?¤Ål#rS?'{bÚs\?ïùQ1Ú}?D Òp-?0ÉÆ9{†?&~Úç;?BVX¥ÄL?AxJ:î*?ïWj˃/?tÅN!x?n®ä©í4°?ršhÍz?'<Éô{ ?™Ó•ÇZ¥œ?ïIúÓxì?{;ZÉ£O?yR–f8?uCþ?lK‡Ü»?n 'Ìz}?ïšÕ1'óÃ?põ%Çú™?c¦&8ܑý?OõðX¢?"a* "¼ç?o,º?×~AGN3FGL J1117.7+0217@p
Ô`ªdÃ@LDêòRÀ:0ªRNmÀ;ʤŠŽcÛ?××2lõÝÎ@îáI±z@9è_ÐJ0¿ÂOØÊã¿äÙGdÌ¿ä"ùiÓÈ¿ßþA†TÇUNASNone?ï÷!/r?I¬«ø°á?>ËCDÏfH?>	RZcØ-?D™Ù8u§I?@LaaÆP?ïœÖŒW3?ˆ*öË9Sþ?v>ŽÞ,ê?|]Íù»í?{ViýueK?Žxo"°®?ï")šD?†Ã.ێZ?ˆ\óúLÞ?zVB±õ=×?r<z³0?¢ÚaÀ!^?î¼V™®!?•rþ³Ç?…Îk¢)Nó?@º"jÍ?öò;üm?'¨èFCéá?ïû:r[€ô?CŸ¹þ¬f?4&ÂN-ç??út>#F
?2ª.§"?1'Ô?ïÝî2M/3?kY08#'b?^ÿ•½
1'?ZT¹°?b'ùeüC?d'à³åo?ï‹:)WÎY?z²ºbÌé?|ík=9Á?r|'=¤©­?}uùRnd?q"Ïû2jP?ï·C¡üzÌ?s`úY±M?pi)ÁØ|?_

AJÔ?sõHéÑ´?nÞ~%vé`AGN3FGL J1119.8-2647@qmMüã@?ÂÚ/­mÀ:j<?KojÀ;ñÅ	‰ì¿ÆÔ_ï @ì;›ât)?ýSwê"¿í\B_[ö¿æ&+7]±®?ÙûHñÓ¿ãZG'öjUNASNone?ïý›¿^?/n´å‰"?¥Û4/Î?˜ªoÑ8õ?3I­»Ì¯?,ºUGö?ï¬<¸Ý?"»·Èûÿ7?rÈŸ8?xÀ
àâ<?w¿²D¤·g?{Wv‡x…?ït\¸E_?zÇ.E'ÿ?xPŸÒ†0Ä?j½Ž£úw?†Ô˜æCÕé?tÛôñâ?ïœ{Ê¥?ŠÓ"ӊC?7ª
<«?L5QcÔt?ˆFÛË\#0?ŠwÂ}eÛ?ïþ''t"Û?4ƒ4Ïè_?
òûøƜº?‡–Y`? ZåªíÚ?£w&ÝV?ïàÍ5äy£?hÿN6¿8Ë?["Œ'D?Vž¼£ÉÆ?ap'y5ƒÂ?b,?öÐ\?ï¶!ö'—§?eD'õ"Ñ?mZÒÆû>]?WŽìwÑ›?vA›E±0?]ȓÂÁs?ï픐pP?[Žü¬š?6ÆtÞÄ/?=/ÅQ¢v¢?_%A¸ô.?WŒ4%AGN3FGL J1123.3-2529@qpö@c^@@¡˜¿pÀ:$€èȬÀ;ȯf•¿«¬"'µþ@kÚÔ¢Y1@Líõ®˜?ë+Uæïì¿çÙi‰9²¿Ø΂‰ÝŽç¿éxuäw})UNASNone?ïÆaHå«?~ȑ 4j?oÒ±pÙd"?rY–W¬?iÌ;Hq+?r‡-úݛ?î®Ê¸šª?¦"ÃÉ}hà?•ßÊyb?›ß±¶-êm?"G2-I›G?žÉQ™?îÇ]L6d?˜ÉÐs¡? `ÝZK–{?'Qé¸?œåY¡â~?‰æGzÆxR?ì8€eĕ?­ƒÁ'lÐ?žtÂYQõ?•ìP9˜?¶žÌQmÝ?©ø;ÊTñ?ïîkQ¡w"?{ÇÀûˆ¤
?Q"ýUf;?X¯7]v@?Q¤_1Ê£?w—¹trD?º®£R?ZvÕ/­ÿ?|BnM…+?ƒÒúíÖ4?yå¢S•?€1áŸýÂ?ï•q?‰âú›=I?«x	4?"&ìòôl?‡žÃÛÿž?y夼çÂ<?ï!«NP?‰Sy:-Â>?'þ‰Â½Ó€?qÒúÇžÆ?'\åÅRkC?†)ÂâŒSjAGN3FGL J1123.6-4558@qö5ü;Oa@,y‰7KƨÀ:1íÚcŽEÀ;šsîå%‰¿mYñäv‰@º\JØw@Žc|?ïýFýå¿à¹f™ù!%¿ë\D¸Ü³?°â×Ö¢*æUNASNone?ï›ðâçÒs?‰>)ánÓ?|Ÿu2?ƒl2ûÏG'?uh]¸Üš?yMN:i>?îo|l.žÆ?µÛígç—?‡ÀºI4?˜w¾Q3ú?£
ž­s?²†¯³Á¡?ìôcT8;†?¡bpP‰«?¨d¦÷æ?š¸~Éûo?¨šfœÃ?"p	cÄ?ì+²¹ƒÍ]?³³NôË<¬?'Ut}_º?ŸŽÀŽñO?ºÕ
o+?²eT^û-Ë?ïå@¹%'?mÇý'4óï?XTrxŽvA?dÏê(X?]*^4¦–?`7 kFª?ïœ5Ã[^ö?"â4ò§²?n_œcF£?|!A)|6n?Z¨0o¾?˜YÉ7&?îyD{[B?"yGÔî?˜ý=)—ƒ3?Êëåۀ?—Ú3n•ª?‹>*HƒŠ?ïO'^Nûø?Ž‰l¼Á?dîrtÇ»?fd"6ús¿?"}Eâ¨?ŒÁ"W°DAGN3FGL J1125.1-5803@r;N…3±@S¼Œã©À:RT`ªeÀ;9,G†§O?åu5¯—æD@
↏-?þw€?*¿ïìꏈý?ä<aëyÙ?™©¤/ó¿ÜêUU¿FŸUNASNone?ïq±Ye?'6ÍŻ·?`±åFŒ?_£!6B?ˆ§+ݼO?'}ø¥Ùóñ?녤ق"?ğ¤ÿ
"?œT~ob1¥?¨–¬:—<?¼½¹š§ô?ÁÚ¬<0Ý?ì½â§æŸ˜?£	+POs'?šil¢† ?‰ÏÓ³?³v‡c| ;? iŸ¸¹çº?ìñ3ù¢?¶t®.7\?ž`['59? (×ð¯dŽ?¸nˆèª ?´…-Çé'?ï¾[>?Œ²0?Lök´?L_·–y?}W'çš…?‹¦{õÜÊù?î°©%Ü;2?®~Ž¨R?¿Nn~áþ?hºÅ†Œ? …šäÆ]?¨aÞ·É*?î·!'—Žõ?'€Nzÿ~?‰?Dî¯f.?yÎ%6K8´?œ|+Sþ S?Ü<(ä?íý½ÙG?žN¨.²Åå?ãxj1è?ÿ§«Û.?¡2f2þžÆ?–Œ..ä|AGN3FGL J1126.8-5001@rҝÇ%Ä@%1uÀv}5À9¢V[LÀ;Œ•ÚÈ8?â£ë#î^@
 úS˜®b@ht`O $¿èµBÙ¿àÑ3cښì¿èAÌsê2¿é¨ó8hɏUNASNone?å'Ø͌m?ÈR°7QG?Ò4ñ¬Þ£?ÇOåGºK7?¦Ø˗D_?©•Ów?çF+Xxa?Ë%õï4?¿Ã¸LÉB?»è•7+²®?Ãvy%}5?Â¥°—ü¥F?ê±ÂaÜ5m?ªËÛâ¢?³†QKù²ò?Ÿ>	\|>?¶ë›£lÓ©?¡Aãî/%»?ãZè?²­ïïx?Î]øÃSZ?²7¦Hw?ÃaÚá ?©{¤"ª?í™'
4?´zü0λ?¯3»§+È?±¡@çůI?Œê­ËÎ?"ùUõ]˜??컐bÿK?¾Íô§ºÍ?¨Ÿì|½?°+5È?Ȏ?¬F^\wgO?²¢µ™vÖn?îLՃ¦Ô?"}ÎV~?œ•W¶7nˆ?Œ.¾©"Ã?™Ï÷Ô¬L÷?"Î÷\ý?ëmïsY­µ?œ¨®Q?·æê:ç?–#\"ŽC£?©S4Yž¸Ú?'2Ä'«£YAGN3FGL J1129.0+3758@eõ5¨Xy>@Qf&,ºs.À9€E¯6¹ÐÀ;|išÎM?î6oùÀ©\@h¬¯Kº@N•`Nõ1¿·ÇúË¥À¿äÑ/÷®<¿áú6Æv؋¿ìuƼEÊUNASNone?á"ø¨rÐ?Ç¿ÁÙK,Æ?ÜvÈ\-[?Çþ`…ÚS?"Ï!<½U?‹·ÝCÀÞ¨?䤂Φì"?ÌiR•Í?њð)PäÓ?É
^u"¹5?´p(æÎâ™?³sV,ë&?ä¤.Gˆw*?·¡·±n?ÒîE?µJ{
d?²ÀŽy¢×?™ë¤JÄì¦?Ýa
~Fç?¶íx~Ùß6?ÚiU"ù¼?¹¿Ï@ø÷+?Àk9ûµ~¹?®!Æ4"k¾?æ­ðڄV£?Åt糂ùÅ?њBÊ2œ=?Å=ð&$Ç?¸»Ù?…j@Tr·Ç?ê±J¼M	?¾éeî;2?ÀA­÷kÿ$?»4½ï0Ç@?£äœ^[Z8?¢G°)Rd?é×XA¤n?­*f£%ž?ÃÛ"rhÅ?ªaûÝô?£õù»?"	.ÖÆ?æÊïë"j?ªäX¡Û?Îÿ掮Ñ?©j¿
ØÝ?§Qg	{3:?–Úèg‰±WAGN3FGL J1130.7-7800@rª"záG®À/ 0 ±»ÏÀ9è<ʋ©íÀ;ƒÀü´ñå?ëe-žÉ¯6@½~Õ(Z?ûØ€nz\¿ï±Â¦"e?åv´@;¿¥šŒéÊîØ¿ÒùHápGçUNASNone?ï¼ì[Ð?¾·3Qí?`\<'ãÉ?]ܼ­êN?yòÛÃJn?|.º  Ú?îºÖq«æ?¨ÿ¡5;Ã?…±p±l??'LXÕ †È?Ì§&E#?¤¦<6´iv?íÂ
ïµb«? <gN¿?u‰ÖX´?PÛÎ6H?¥$\ (ï?•µb©Á¥"?î9;»B?¤UŒWõ[ø?Ž…v.×ð?×¬/æ{?¤Í¼F?¡ùg­µÆ¦?ïØ­|ê%<?p-ˆ^>é?Tp‹"M5?R
‡¬wä?m=ƒò%?kfÆ Ëӄ?ïÌ›=wt?‹íc¯Í™™?j‡"U$»?mŽsyËN?êøb=¹?†ÛGˆŸJ?$‹"?‹ÔeÁ|–ç?‹iNâ¶û?~BȧG±?ºú?'¯Z!éÇ ?ïFÉ:ú…u?†lÅKRy?ˆaX|Ç:Œ?zqç½.@?…ìXėh?}¤GS@æÅAGN3FGL J1132.0-4736@rZ¬1@*SQÞïåÀ: @‹áJÀ;´)Žnÿãê*ÍB>@±§+'¡@韍#•¿ïþž-Ò÷?ïÝ[Qy36¿à¬¤±®@ù¿æ3²UìàWUNASNone?ï¹HòžSÏ?"\c+"Ž?_T
 Th?e_¶i³?{†ƒéäG®?"éUnœjÚ?ꓑ6J?ÄÁ+¨i/?³('ϸÉç?µÈÖx;3?¸:â&–»Å?¼c8oÄD?îÉQ(wÕ?–ÎÈ4ªr?"El³ã ?"ŽCkaè?¥€´àæÂê?'ªÈ U;?ꑈÄñGg?ÀË«mV›?À¶Ìiiië?Àf¡Ó,•é?¤B
ٖç?¢Ú;ê¾È?ï݌c·E¸?•<(¦ò…Š?@Wgäˆp?B¶ñÝíl?n]ÂBÐ0?•5BKé"?î®qˆê†?«öÂgÆÐ?'å%ƒÿÖ?Ÿ£2ØA
'?˜L©^°$ü?¡	ò–?ï1PiœHB?"œÏœ'†?"2€O*"‡?w>ìæÿó?yePú‰î?Ô&5†c?ï:J7˜?°ºÐÿj?‰2(¯I*?‰WúÔ!HÞ?ˆ&•H¯¤Ñ?ƒjâ‡Ù,žAGN3FGL J1139.0-6244@rkî¢	ª¤¿ðZ*~…À8%ô¬å§À:…"_u±]?íä+¬3ب@·õ$YÒ@2^ÿê±d¿ÜSä,©›¿â$ËdÓûP¿ã1O¬Té¿êc€ò†UNASNone?šBï5Þ?œÞÓ¦0?á°^4Ç;?Ð7˜·`BÐ?ÜLpQÝÔm?Ð<çðrL?]j$"êrL?utò|©Ì?ÞQu"'ÚÊ?Ãÿ>	â@?àȐ#gýÚ?Ä«ÿ!ß?Ì*)ê_.å?²©Ã"@õ?ÒfQ,1P?²¼ªœµÔ?߄™ß±ù.?µJ¢ÝÝc?­7+úÕÁ?œák¾Š­?Ùtá´E?º˜WݦS?ár‹OÿÇ¡?¼Qýù•'´?´2I3'¹?´¥ýzöˆ‹?àLnB¨Ç?Îè…SÖ/¼?ÚÒÔ×:ío?Í«8Ž£³?uTü®×6?Šb
àNvë?Þá*»ŒÖ?¾ç«N¼•a?àeC@œ}O?ÀBe'e?଀ø®q?¶ImêE,?È`£³ԃ?¬U§œ#¨?Òv¬6K¸Ý?²¼Çeí‹,?º·[ó%*?¦ 6POø?Øö1l¸?±/ÈN¼°?àš™i$ÿ?´ƒÉT˜BMIXED3FGL J1142.1-6941@r\|ؙÀ}¾Ý 'À9¾±û.·À;:Æ/#Ú¿Ú®ÛÌ*K¿@ÝX›L¢@F˜ÿÀ¿ù¿ÝnŸ+:&©¿è槍çÎu¿è(Aš Ÿ¿èŸÈ,¨LUNASNone?À©(?‹¹ˆ2¥*?qi™ü\Þ±?v4'ð`ï?ƒÄ'ž$™?‡ K"K?ìÖ²'ÀK?»fÄÒy×T?'.8=,]?˜9'Ê΅?´¾Ýgºÿd?·œˆ|êB?í$G­"¡ˆ?žb½ùðþM? ù¬.많?Ž¥Ö­
h?¬ÁØø¶&ñ?•£5{óý?ë`¤^³X?¥€Bû:9?'amD²O´?uødm¤[‡?ÁYâ™±E?¤ØÁƒ;¶?ïÈàþv×½?'™\9t:?[Ù¤7¶‡\?^ŠË{¹Ý?t™›) 
?ýHÚL?îøu²)?£Aiúí?zƉMv´?~gÃφT?š?» z/? K¥
Š\?îözž,P?‹µÍèçÆ´?ŒdÏQPC~?}Ôß^(Ž?'þU`"¸8?"lTË£?"/"?†VÆ=ð;?i"`6Ëgù?U;Ü°]Àü?¤¬Ï]˸?…žÜä÷[AGN3FGL J1146.1-0640@q8Œ½D¦@JWe<š»À:EFšï/À;¼ì÷À?å×r%?Z@éeß­Ð?þ»È?õ8|¿îZÖ×"ø9?ÉxLÞ¼»¿Èܸûè ï¿å 5j%UNASNone?ï÷ÜìXB?FހÙU
l?B1¤4I«?<éoË5B?<µWԃc?7§ŸøHž?ì>²4gˆ?¸—£míi1?´ªŠ›T?³ê¿:¸Å?¢ÀÛ£yœ?£"Û,yE?ïˆý?ƒ[¹Ó5¢?"xl><ß®?q	éÛtß?"Jg?D݁?|ŽC/˜´˜?êÕ"[ʁ?µ+Ҙsß?¾·+áìTä?³•áwÃtÎ?©"VÚJ#? 6…Ôéò?ïûðïÊ[a?3D•±>JÖ?,ÛÄ/ó\?$×,²"?2
÷Èe#ø?(NîÊà*®?ïUà¡?™êb±fo?"x1gMÑ?":¸§j¬`?…Œ×çH?"ÿç[R?{0^(?nPˆ€-?xjòöO?`¸®\r:f?')¨,Eä?d¿cqZ?íTø}³<¶?Ÿ8ÌÆL?²-T™?œ«<?‡"?Š@x4&õ¤?EJH‹ÒŒAGN3FGL J1149.1+2815@i•nÖwpz@S¤i×4/À:JÊ<ϔ'À;Ï#K^£$¿ÎþŽ]GÑ@¨¹ù¶dÖ@©¶àQcö¿ëÂ`?äO¿ã~œbC8†¿ÞôRds>ˆ¿ä®àc隟UNASNone?ïñ¢1KZ?YŽ‹ç[ñ§?@݅<K³?Cˊ×G0!?UeøדŒ|?TÒʤ;Ò?ïsj¨6ã?Œ½EÇꢼ?z8]DØ?'òtžÝ?+U§Ã?hÇÍ2u?î ¬U¢?8<¢ì«D?šòíÅV;?{Œ"¸?
d§?ˆ»'è¥?ï]E'•Ð?¡©È7?VT(€ç™?uBnû€?—~ÂJ4N?‰•Zª!zo?ïûªW¤N ?8cß{‡?%ŽÍ""?"Iþ:N?8%ùI€?3€ùÿ•"]?ïÛ1Ò5?pŠ'Š"Z?`ÿ•Þ¹]S?b˜ ("¦?cΘͽ[?d݉gÛ!?ïy´i~žÁ?xØÖs¾5?z¯/¨Á?d³]ªË@?"Ž'öi(?t䟐‡u?ïËÓ·'k?g%ô&°?c¸‡½nv?Ps|Oµä?p9àt?cP%/°	AGN3FGL J1150.7-4816@rIø -à@*½½×fƒÃÀ:Xóz¶ƒÀ;¼ AS‡g¿Â
ÎʨÛ+@ùÔLfá@¢ÿZcN?Üù)Ƒ¹¿åՍÌÂø¿ìÛ·ÿ¾Å+¿¹Œoôág.UNASNone?êPÃV×R7?΍þI¶F<?´1¨ý>µ?Àñz©òà»?¹H=:mñ?ʂr*êºI?î@%Vs «?¶·Õ‡?‹sì#
Òû?šŒd9Ößw?¥ ¯'ÂNˆ?²«¯Ôk"?ë©(tàŸ	?¦‡Ru;í÷?¯
xØ}Ÿ? j7ȗ~¤?³1€L2áé?ž;ÌßÂð?ìµÙÞ® º?°#ËTZRå?Ð8?¡%‹?š5X+'?¶"ü^~É?®øja'?è1G¸ÑBR?Ù¾ôP¹Ö?§À¶uÎ9?ÂtûƒÞ5D?ÉJ³€S*'?×E¿Ö±'?&.P?•¦öÝ,]?pDzÒy©?y=\»ò{ß?ƒóy'ú{?šï×2"?îÿÈ¢›¡?—º[ùY7?Ÿ)nÌ,$?'©b*´?–˜YÈ?Žeù¹QáB?ïr»Yr²?†a;c–Bñ?b¤ÑþhH?a%~|û-Ô?Ž§õ(ÀÑ\?"Í"¦Å–AGN3FGL J1151.5+0957@pJ^~¥øM@PñŠÚ¹õZÀ:|ـ9vCÀ;âÍ)Á¿ö­sU¸`@¾_ ø@Ŝ@Ô¿ßےêË1ä¿æ)jÀúAá¿Ü¡ú¤t¿è‰¼qOUNASNone?ïÖX]|?v´Bì?Nq|é´?QEIa¦Í?q°…yÀ ?t:Cû?ïªáü›à?‡
äIw?sb"¼ã*?}q]wî»Â?wxŸSÑ
?zõ(–Ž*²?íõÕÕ½"Ô?œFœ¹¸½?'ñ%M?'"eúf¸?§ªÜ3?™»oƒü?ïxO?tO?ƒðm^91?RÓû=ñ Ã?R™#>ÖÏå?'°ÛÄP@?ƒ)˜ŽÜn,?ïõü/¹8?V³hû:?3S*ªj!?3àå‹'?NeÀæëV?T¨!Z
h?ïä6ý(ps?g*íƒ??Y$œR¿É?WT˜¾ìO?^mi_Ì
³?_Ây÷ç§t?ï@|3¤"—?…:_yØÌ?~¡Ó%¶°Ç?kÔ«ó¡=v?HÁÿÀõ?ƒ,­ŸkXÔ?ïè>)ã:?[A¥¶æ5?+†wxzb?%®±DÏ?f	}ƒîŸv?Z†	8ŸÃÿAGN3FGL J1151.8-6108@r|Щ*0?ìʏ۪¶"À9	ï]ñLßÀ:ÒFfޏ?êZz%q9å@ðé‡B©ô@w†ß­¥¿Û?€UrD¸¿¯;!îV#<¿ë#Â2G®s¿íÔەx³×UNASNone?¢{eò'?©ÐøFnü?í»Иx ?´î‡7Ø?¡Ô'>Cx?ª‰Ä‰å'?¡SZ΋F?³S™™¿eM?ÕñÂk† ?ò>mÆN{?ãõ9"	<?Æéî†0V?ÓͤQó,?³×{¯&]]?ØØ3§f$¼?´=;%Ä*?Ô%þ´Gè?´"c	7
?ÆϞæWê?³À"Â/À?â®ÔY«d?þÊ5mË
?ÎwýÈBN"?¼»¸Ûܽ¹?¯àH+r1'?¶hQ‡"$?ì6z¹À¼¯?¿|yo¤õæ?¬¸6Ê5|?±%pövå?°UÁšÂù	?ºO)çb­Ó?Վøî`<Î?»"?¸QÀ'?ã-ËUåu÷?…¥§?àDÐÀˆ'?³UË`"~ø?Ó­81õ›?°UO=°Ê?ÈÛbŸÎE?¬ƒ$™.¾?Ú,a'?´oîÁ½oÐ?օˆ3{ê?·ŸÌʯ¢?Λ÷Ø>E
?°˜Ü6Õ³MIXED3FGL J1155.3-1112@q˜|ßýa@H©>¢Òþ?À:ŽK†ýÀ;£1ßÈR?ð
ƒ® ¼Î@`þWN?øIúÑÃ?é#ÛΌ.f?ëšG>'ó?ç(fº¿ß/DÜRü§UNASNone?ïÑçc{ûN?våëÌ«5—?cÉd$ÿ&.?dô $M?jO8z'k—?oJ±!G?ëD[xyN?ÊG_Ù(á?¼*ÎúhUC?Æk·½"k?£dªyº£?¯–"°Å†è?ìÃAå—bÌ?¥å-ÜP0A?¨ËL2ø?š?B¡jg`?«ÆÆÚa¹B?"»òɆ?ìç¶En©?½Î³½?«jœSxÇ?¸ù Z
©?¦ÿVH`?®å©_B,?ïÞcî<D?qY—ð§ëg?[7hAük?\ T™ÂVÐ?d]æ­§?i$´[?ìÃ\TÙdú?Ä݂`±µ^?´?rr‹?Â&šø(?—w¡êN}?¦c¡mqŸ?îRG4Wd?˜E¿Ÿ4/ª?™sÑIcj@?ŽWÝ\sÆ?œC>Щ4?¢c¸NJ?îQ«vïS?ªéA=?©:
÷V˜{?§.ÒcU3?"Ãi3»½]?‹¿ÌkûgAGN3FGL J1200.4+0202@q-¼U†D@Oq²•êÀ9ã£v'-•À;¸îA'šÈ?ß	袧pƒ@#æ9/w@H½§Õò¿çEÂ[H"Þ¿Õv.­3÷¡¿Ôc)ÖÖ2¿ç¼*¥ðêäUNASNone?ïó«à\æO?Rý3ÀIxC?PnŒ`…*¿?P
ªC–"?@sf&ú?8[.Ð|š?ï%?êsP?"q<™b?ŒÆf¨ÁÚÊ?†ÏFjº·?‰éž·5 ?Š}¿2*U±?ï^×
Ãb?ª±<#?€˜§`ì{×?r«­"3?‡±•>	2Ö?s«w}"W?î.:âe?™Ð8ÃêÓ?›ç§XCïá?³Ôu'Y? yH§tß·?'[\ìò˜?ïûv.@Á?8q•AÕ*·?5ìì_`Ó?3Ž®FB¾?*NÅ
¯(ž?"7ÙOûI?ï¹oèÄ?vfB
XÌß?r¥KÕ}?jL¿Ñ²©Ò?p£	âin?mø*e´x?ï­WÍ,ª?lޝ/bI?s$ßâÃùþ?e–ÐÝàì?vRô<ÔüÚ?]c{
Ú?ïYp>½'?z¬J\€Åž?‹ì#ôÍo?rFb⻳?{˜õÏì?nÀF$ò¿AGN3FGL J1200.9-1432@qÐVÕϪÎ@GHw…À:NÌ7«hÀ;¶­¦–Ø?Ãwx'7ûo@ø,*€\1@)«0ñ¿íŽä["ª>¿ÜI6¶† ¿ÎßÎÅ~–¿âVÎÜz"UNASNone?ïü\:úl?9~'
û?2ȽϺ"­?6Лí;—-?$­"kDcB?"jœ`~?ïŸJ«k‡?ˆ·;:õ'•?vQ•K¼¤?€ÔÁx.ߗ?z	_í«àˆ?~ù‹(ˆüf?ï%b@©'?†å1ŒXØ"?ˆÝ¡žZO€?÷-2$'?ÉÎlir¦?xïÖCÆaÏ?ïSØbé?…?‡õaÈEIM?hì†mnJ½?i¬ï
ª?'gb͛"?…­7ÚW'ò?ïýá™ÚÔo?(ŽÏ€¤1Ð?%XP$eÌ?%âïÆÐ%?$R¹Ÿ?Eœc›‹ï?ïß©Jfß?i]§~sHX?]ÀÔµ¾,:?W"ÔÔÍ´?avzŠÔ'?bÚk©@à?ï-îÖH?uÕü.åʸ?x)ËäÆé?qw2ÿk6ƒ?y?ª»,Þ?c9ó; ?ïÔ»Ùq?cÈ}-bnÌ?_ď˜º"²?NÖ01:>ì?lœj
?_ÒK™>AGN3FGL J1203.9-1745@qó\=îx@EÓÊ}g3ìÀ:R·*¤yÀ;ק jٓ?éð¸Á^ã@ù½',±@ZH@5¥(?ág6s|¿Ï¡ò3Â-¿âýÕÊ2¤Ô¿ïÿ'wJUNASNone?ïp
ã²0X?"y@	,?'Yp\ÿø?">‹
r9?M½B'•Ë^?NïEÍÖ¹‹?Þíº‡i°?ˌI ™#c?Û"³*±§?ÊßYŸâ´?·ä‹Ғ7?´8%8pJE?ègbfôÎ?¯ùwš~6‹?Ç)ªàá#=?¬z›†õ?¬ã.
x¸?šlú?Ý¢§¤¸ö?¿ÓŒUI™¸?Þi<â ?ÀÉ1:`'?¯¥*'õR?£»¾C³c8?ï¤Î´¦x?Æ«þÿ'Š?"ù_áü?wÊÚÛ·?M-N&\?J0{F¦ Ù?çÇ¥S"°.?Ã
ˆÓê?Ê[H]f"?Ái¥†šR?ª‰Q·}'?¤[	ãˆÅ?ê˜ïfÄsý?ª'—àkl?ÀÄn0¬''?¦EÔ¿m:V?£_PÑuî?•2Éé´[?é"yé>â-?ªnRòTìw?ƱK(¿´-?©]9¯ÆÇ?—æi"g©?'¿R›`MIXED3FGL J1205.9+3315@fGohی@S›Då^³À:WÌ¥_ À;èÚ'QU?ä¿ÃôOâZ@
þƯâÜ@·9_‰¿íøÔÔy@¿ÞòÇK;¿äÕxÔ
o¿Óý™üÉrXUNASNone?ïñß̌h·?[é‹Ó=Y?Mô¶‡þG?SÙ~5ü ?JŒ"EÛ?K"'I…3?ïnkŠãÉ?˜2|ʘú?€n
Þl?UFöŒùH?ƒ÷0ö€W?‹ÛNù?úõ?îA¯‰U?—;´!Š]I?–Æᅩh=?ˆ¶bKPj¹?£xtEw-‰?'/X¶˜?î"er­?¦¤©R€G¼?¡#¦‰Ó'?¤ØÉBDA?™uçÉ+E?'øF"±N÷?ïø'ÛºPs?Mªe"ÕQ0?:ˆ®K±	?>Z`p‰í{?@tͳïÞ?C*Ž´I?ïÑоZ)}?|4ÊC!ì#?dƒüÍ*?n)«33Ê?iž¾¬V•M?r3/8o
¹?ïBbZ_"]?"›XdÛc?ƒ^ltV?x,™Y ?‹ØKet?~¿šbSö?ïë¬ûó?ƒôæ5·D?"ëJiÚ?€ìªNÑ×?ng*i\¦N?m&ÅIEAGN3FGL J1206.4-7123@rµ7KƧðÀ!®ªm&tÀ9ƒ@ìYZÀ;k8$3»ï?ê'~~@%¤ÝD"/@qM éÀ¿è'½{ºÐ:¿é8úž}jJ¿åÚ´¼Dñ¿ïÿ¹ý£jUNASNone	?è	ßk¤®?ÆUåTiJ?²}ºáþ/?µ7oRÕ,?ƼûÛNñ?Â2
™E¶Ã?ϱ´î^ÂÙ?łՒ™K?Ø`›''?Áx6äSã=?×Ɖ÷»
?ÄÒo®¹'\?ç{`§\?´&."Shå?ÃëälH ?®$Þ¼Ñf–?¿¤\"7.ã?¤…7ŸÄúó?؏Z"
?²éÁµxŒ?×k&hŽM¥?¶<ޒf?Жc.N?¯Z­sá¼-?éeìGUBì?ÅG|L.Ç?±¢(Í«N`?³ñÑ|X9?Á—:{žS_?ÀÇ
ôƒS?à± žðŠ?Êi¦ÑRà?Ï	(ä‹ìn?ºñ̎
Ÿ?Î2VœøQi?Á´ýÁ?¨?ì~`ÇÚ¹?¥p{`pœ?³
 –'?žœCSU?¨ÿ´5E?""[?äïÛíH³?§øø†±Vò?Í͚K´ù
?¦&¾O™`Þ?¼åëþQR?œU×GÛþòMIXED3FGL J1208.0-6901@r°µ^ñýßÀíäßé	CÀ9Úe;ÃûÀ;hK!f'?ç'͌\½@
¾öJt˜@ÞÛÿo·H¿ç¦2™°?οã/žùÅ¿åÙx(¨F¿ïÿíK¥ùWUNASNone?Ó(Ÿ3Žð?È.§Ùßk?Ñ…›µÓŒ?Ç
U¯p+È?ÛÔÛG"?Ío¬Ú­ÏË?¹,þÑ+×?¸bvRï?ÞÖ´vXª?'3oOý?ÚÞÕ\y?Ú_<P"?äÊnÓiÁ\?±í²¤YE~?ǐ
,\]?©õ!@Ââ?ÅF:…ü?«€hê&?Ó|‰éMa?²a܃ÀÖ?ÝlÅ6fª•?¹nÍ©q?Î-aÀ—èÈ?°HºLû-?Ý\DR.?͌r¬<Ué?"wªË4
?¾eÈqHl«?ÙY€(H7k?ÍaT½¶H@?Õ#–F—­Ë?Çw{"ì‹?Öëu²éÄ?¾~°…Õ}²?Óðô³µhq?ÀØ[YÕÆ?êRpK—ƒ?¨ÅY$.?¸Þ‹2šÿB? ÉL*I+w?´'KD¦? !¿üÜi`?âªË2mæb?«‰ÊO·%Û?Ò? Ñ"¨`?¬:ò1Â?ÀՑ"!¶? ;†­vbMIXED3FGL J1209.9+7607@_Œìk΅4@D^™côÏÀ:J¹¥¨œÀ<{DD¿Ó4ƒÄ‰öþ@
§ÑjÁ?@/`œwð¿å–âcâÓ¿èësg<¿Ñ'Û ïÜ¿í>vÒçjUNASNone?îû*DН?¡JD_¿þê?Í7œG ˆ?˜š'y»?›À‹kœ?"kÜxæ?îS@fCù!?¦Ë×@""¨?žKDã9Ö?N"w'?—L®PØ,?š¦_F—?ìUñ
'ð?£¿ä1 ?®oþÞ gr?™0a"šÓ?¬0ðwq²'?—	ýeä
ñ?M6г?™ãT­?‹·à`æ:U?Š~ÿåSƒ?šò¦%C0?"|=mgÅ3?ï§ÛëðöÅ?‡…é¡_YÙ?w^˜5?{UÓö$Ž?tõ¬Y¤?~#RhKÁ?ïŠO5§`?",‡ÃéY?€W¯þ‰Ø?xÍ Zl Ñ?z**"˜E?wƒäëð[?î™Ëm§"?•¶Ô0üôž?£Œ±ƒî?Ãñ9œ6‹?˜Ô")bÛà?'Ûä¼ÿ?ï¼úÑÓ?s¤U¯î×?pÒÜJ2?e
Ά —‰?p¯Ôà<Ï=?kpJÐ9½AGN3FGL J1210.1-2742@r>ýuâ@A"–'§\ÑÀ9©±¿*À;€8YáÀÔ7cnU@ë&šž|W@¾Ç :ˆ¿ç­U™c¿ê]hÓþð6¿ØR×	Þób¿êà‡Q:UNASNone?ïýUT+Œ‡?3|A´,âÝ? ¬•0¨? tÄsão?)þBjí?.*‹æM½?ï¹åz©Ð…?†ä xçå…?lø°PûP/?w†n藸×?têql	¯?W©–†#¤?ï¨	·'?Œîôžä?…–­7""y?O4K"3f?"¨4o¦à?‡Ž¬" a?ïÔٖ^ѝ?t͙#C>öªnz×?'MP¥?u|ŠGr¬"?tÃHþV?ïþ³IÕ?*§-`üK?#9Ž¥ì‹?%*šËÿM?7'·RÀs?&"ÞÙ¿W?ïæ‹÷^`?f…ý¾-ãî?V*e2π?S(¾zx'?]µ¾*'?`~j¬Ú³§?ïjë8aŠ?‡þ€©ØH?"m$ZM4ƒ?"ÔlÕö?
 á'Fæ?wˆ•ŠD{?ïø`.`]?Jù
Åd">ÅÖ.ïP´¯>Þ!¦eÜD?OØ©'{?JòLAíAGN3FGL J1211.8+6413@`>ŒSâÖ@J.VCæÀ:Ì-–;@HÀ<3¢¾‰­¿–Ü,ïªÑ@
%›@xqû¿í¶âyÔ¤ª¿ÉƒËÒ{¿æُŒê"¿ÜœVH9UNASNone?ï-=-?£("7zY?˜ÄAVð#T?£	vyË<?YAm	?Y¯°÷J?ïwø²âH"?"¶3fKô?€´uxâÖ?ˆÒO"r*m?M]ÖrÜw?‡sšÂ¾Ÿñ?í	°$öYŽ?¡òŽr1g?«HJèŕ?Ÿ(8Í3Ìw?¤²Å
?]ºˆaê?îýãŽÁ_—?'¢þ'§Ù?'
ý¸ŠÈ?Œå8L¤RÃ?Œk ޒŠ?…=
ó/)?ï˜~& ¦?¡a	€|2?ˆ‹ï‹3gp?¡Y?Õ»·?EHoŒA"?Bå×DPæ?ï؁'MS?uLe^Sa?büâ?J¥?gÌ€"–$?d'[¾Ýjé?icpªÅ?î¡Ý·o‡;?–cŒ.†'?ñV"Ã8R?•¶ƒBÜ÷?‹¥ä÷($"?t>š›Õd?ïÖÓߙ5Ï?ig"™Á'?hÉwöæ4«?[â÷}C?`b¨à<?`Cµð½ñÖAGN3FGL J1213.9-4412@r~Â&€@2$Wâ?$ÙÀ9›Õ¹ÛÀ;"«² Ñœ?¤63©åv@üW-
E@'§_ÕӇ¿Öaé0¨
î¿æázéÞ´¿àsHš(½¿é}œ/mxUNASNone?ïÍ\!>6?s¿"›Ô"?qvøŸ®o‹?q{÷‹:?_kڃî†a?[쾊äÒ×?î…*Í;» ?­Ïnµ¤)?'|í»»Ë?'Ì.°ÿ?œÞ¤oôJ8?¨Cd6hû?î~Xë m?"g¾#ho=?–ê›ñ‹é›?Šu'ºh'\?™JF³N°?…©{]A³?ìO4bª'†?¢I&ÉC[?˜Ý!ê5"?†ï–Þþ?·OaTÿm?¡5ûÄÅ?ïò@Aíñ?TOü''o÷?RŠ0e»€%?Pï¢yví?Aê–ӝ©'?<´ å´)?ï…Y©%s?'yi`\ZK?y
X7heß?tžxsFX?'$iƒ1¼P?XHË%!?ïe"<ôŽC?€217¨á?"o—¬ñÆ?yÒÁÒ́Ö?'+Ò±]Ž?m¸vyÛ?ïW7Á°?ƒÞ¹!‰é?"u{@‹á?jWÌ]C,?•ØX§Ô?4a%EÊAGN3FGL J1214.4-2315@r?÷eýŠÛ@Ci/Âej¾À9õÅGMƒÀ;šñ,'¦7¿ÝöECM@

ÛF["@‡Ÿœ¿äšgãq²}¿ç¨ýÀ	ÅÒ¿âB`m†žÉ¿à5\ë_×MUNASNone?ï>ü*ˆj?šõâîíÌ?jm9rŸ%;?hù°¼"<?"ïFÛ®'?™/¯Ò{?ïV@OÀ †?¤¢èýÎÛ?ƒ	™ç´8
?Ž¤Åï#i?‡fR}T•?ž¦bsÎÀ?í^›c±? ˆêí¹ó?˜ËA‡^Ù?"'`yÄ:x?­°¯0•Û/?šã5A_?íÄ\ñüâ?™ÆÃߘue?z8^ýôÈ?tjÑ÷¬9?°9'í±!?˜±dÃLf"?ïã930¿?r3 1¶uæ?F6›´b
Ô?Iüì‡'…ï?g9%¨•'Ë?oØ*mõx?ïϓ.N$¯?vR­¿š?fKt϶
O?g'æsß?j!]¦?nFeìÌ?ï5,Cn®x?€_§uœY¨?'ƒ7>7?kߍ;‹Ë?Ûë	è?xÔ¦5`ko?ïƒtf"Cq?uBþàvÉõ?`<Fc°äB?N ƒ>-'?‹Ô½î¶?sø"\Ž*aAGN3FGL J1215.9-1926@r8Œ?>q@ES3"l;'À:-H*;<íÀ;ºêßÝJÉÀaa;.T@—ÿÀ@Pwߊ"™¿éßv\›¿ãñ¨‹Üë¿Û€Sɱ¿í;=ž¤£ìUNASNone?îÚÆR½Å¦?Ÿø6M"Ž?ŸyAzí³¬?Ä&e8v¼?t·ÐÁ
?tW"îá"†?ï€`.'¹?Ÿ+	Ÿå-Ú?~Éʝ Iï?—•N0d¡À?€ƒh­ò?‰ž0\Ï7?ëJ [®ì?¨f:*J
Î?´ß#Ë{î?¡Ž²8`"v?°Ð2ña/?œ6­7Çq¸?ï±¼®¥"?™;™t©Í?QÿÓë"!1?d¯î?ƒ?›	Ë3YCŸ?˜Æüªë8Ž?ïhê9Ŭ?Ž,O<š?I\Y6?‹ÑrêQn½?j¼ É}{Æ?f'(‰q8i?ïÛÛÓ¥Ùï?y…¿{º8[?`s]Q33<?gÝkcºà?c°ÎŚ†X?oààÄd´?í}ÊçÖy°?šÜ
•J·?¨àñî¦Y?"s='oO?ž†m,V?‰ß$Á	?ïÑÞµ`';?t¼½ú»·@?@èL|Ë?%5u'ñ»O?vË¡É|×à?t¦3ùLçAGN3FGL J1216.6-0557@qö8<òϖ@Kí@$³=°À:o®
ÅÀ;—\>Å7­?Í,Xæ˜ð@ü;û-Þ@Ý0ŸÚü:¿ç½žÁ¡ y¿ä°ÎøSÁÒ¿ãu7	àC¿ïýÌn®'UNASNone?ïáŒ+$¥?e'hî6Å?eåaû8??a÷K?]QÚ?Qþ%´>fe?L$|©ê¨!?î'g¶‹l? mX+¼Ñ•?š´â‰'?–ÞNõôrà?'þ'(\a?"1¡Vµ?íq3CÔ9?Ÿ=ٙ'ȋ?¨w|U"p¶?•×è`†e{? uO{Rµ?&úŽÓ¢<?ëŠa?(?§`ÕF²°±?²W«ßÓ?¡µF

V?±UL?w"ò?œ'»Ÿ—¤;?ïð-ñ;'Z?V¬`b—­?W­¶ª²?RøH^½z??ٝØP5?8Vzí-0•?ï•èf2?çv©Mv?}æ+]çZ?wº¢I4â?w%¡•]•?uˆÞ#ùç³?îÕ«Að?ˆ

¨qñ?—æýV€µà?'£¿úŒ¼§?ŠÇ5xˆ8?tý
•wÑi?î©6ª-‡ð?†¯O¼À`?™ËÒú÷?€öí0gJk?')¦|?|Õæù·")AGN3FGL J1220.0-2502@r_ÍÓØ@B¤!ÀD(NÀ:WfÛl7À;¬—AЄ迶
ˆnÚñV@ŠJ}Qº]@r`Æ%¿ïÆ»y$?ÜÎk6Ʉˆ¿è>)YÉ(¿ÒÈ*Ïj£UNASNone?ïñÃ.hs1?\O²ú¤…‹?WD.s;?[SFLM?4ÖyèHt™?.îýëÜÆí?ï™y¥Î?Œ"Wr÷|?v"³¥[´$?€ÏΠ"´)?}OŒ³Ø¹?"ó1ŲÃ?îÍév•we?)j‡ˆJ?"¦¢-ÌH?†o™WÀ?"6*ŒÛ?êVG?ïB	[[=?ŽÌé3R`?ƒyûÈþ?"ô+¸±?Œ¢ê_·?†M^H-íÙ?ïû>\(—E?A–ùGY+¯?<šö{Ò¨??ܧ³Ã–Ó?"äNh‰"=?Ê9ËÌg?ïÝØïùU?m§'"6[?^DÊÔ1íy?Yw®«+>×?cÕÁÄ*CÐ?f™	¡ ks?ïu|œ°?}ÓPÁÄx?'­=!bÈ?w¡èC˜?€£ý†å?om*÷Œ«U?ïÝ¢¿Õdî?cßÏÁ›V¸?XMY?KÐÛ-òY_?fR™NËã?`°F{݊AGN3FGL J1220.1-3715@rAc@93MjOÀ:š¿3‡À;½ò×"'%¿ÎDn?´Üý@
ää~`y@_ßÿY'í?Þu`ZÄØÉ¿á· "IÖä¿â€BÌ=¿Í]ßØ\UNASNone?ïí¾—TðÈ?Y1¾€¼#?Ad,ˆÊÃv?<€Ô¬¨ý?[к֟ÆD?TÜ}E›?ïŽw³Qò?'ÕðÚ?žs?u[]í¹4?zá2°ÔŽ?´d.©d×?…xû>z9?îè÷@Ïå?ˆÖŽ¶tmQ?Š±{Úä4?yŽ¡"/n?•ˆYõ!§0?'fԜ6Ci?îÆE gö×?—¾Òš3?i´Y²z›?kØ´r4?¢
ò·Âúf?–r3·.Z?ïø§½YùW?Cõø˜Á?,†fâ¸?%"aþӐ?F=)s?(?@ͦ‰ê–Œ?ïØdîA;µ?rôA\øó¬?`0ò*F7?Y¼Oî×?gj¿G-?oUèìrlu?ï}v';X?w[nñN¹?|qOê¡8'?kŽS´ïË©?'i·–9™?póPƒËÞ?ïÇ¡/Ì1®?qû©høq«?K33>¾¯ð?A‰U'3â?xÉ·ø@Ï?qI¼¨
¢PAGN3FGL J1220.3+6055@`4'¾‹Áj@Kå~ºñ6À:ņè¼í\À<  ‡Êd=?¼"Ze@9»n€'@#?¥‡d¿åùáéû˜¿éÙ¼06Bv¿ìv'"×?âK˜N­kUNASNone?ïb=YI?³"ßMªn-?‹&iØ(#?³•wVF•?IØäÑ g?P=•­Òv?︊À?‡ð7¤ˆÀ?q
ÌB¢Š¯?€	z™£{'?rç¤Ã‡v?xM/jr*è?íôa{Åô?¡&Ó¨ƒù<?¥('[Áú? v$
օ¤?—IfAÇX?'¬,µúÉ?ïÖHrÏD:?y…@W›?BÇ%¢­á?\WRJCPÓ?r‰­¤y­§?xE9Y`Ä?î•Þ9ÂՎ?ȎgêÓ{›?¦ÞI¡ßŽ?È@#¦Î5ƒ?R'Âù!²?"u¥‰ÖÜ?ïå*–xõ,?jª2 ;¡M?YUX–«èÑ?]ô£µb1'?\Uzg?«?`*q-jÍx?ï
ëç€h?'~«ª%˜?"
ênè#?'¾X¹×1?"ZðSGX?rFÊÕ©Ò»?ïü;»ÔM?LU°§fÊ÷?)qãoƒ±?0mÅ`Ù/?9Âó€<U?H¼ÞœŒ8ZAGN3FGL J1221.5-0632@ri$ò'Ð@KÆ YžØÀ9b+åaIÀ;'ÍDÁÐð?æöËA˜Œå@±VPÇ!@ÿ"_mλ¿Ý-V·$x¿ßìj…ôù¿áû`Þè]¿îÍ¡¸ÄN›UNASNone?éÃ[mþ¤û?֭ÝYž?È[aƪ°?‡÷ª4á"?rî¼Ì§ ‡?p1h&µÄ?ã|½_"Û·?Îtvöñ?Óõޞ±['?Ë¥ØIá(,?´Bš‹/i<?²:úöØnT?çeXÄ^¶'?±ø.a°?Ëõ³U­[˜?°Ow*#­?©Ó¦eö‹?"šyñç-?âÍp\ù ?¹W|à°µ?ÔX±R%ù?º+ûñÓly?¸1¹8y?§}Kéº"¹?ì•O1kˆ?Á›Ì hQ?ºžP¸7ï?ÁšpA ?g™Ìkê9?abßZ-qø?éÞC'z ä?ÂF·?ÃJ扝‰O?¿ž'Ìùmj?¤ð3g6…?¢‹Ž­Ç?ꬖ$U[?ª>•v{/Â?Áy){hDý?§YÖҔ?ž£ï"3>•?Œ	µæuM1?êÖ°¶k·^?¤C!cy?À³jˆŒd?£ÿnԂ?ŸŽ"ë¥y#?'T½[AGN3FGL J1222.7+7952@_ Ò
ú/@B–-û¹À:Â3|.NÈÀ<%K#É¿è}ê!Ø~@ÅXlþ†?ûËÓÀ±ád?ïî·JÚnÌ¿Ü&¢¡U$Ë¿ßrøËXX‡¿¼ÖçzDŒUNASNone?ïðwʚv?^æölIÿy?1W£Hgz?*¼Fæ3:?Zº'×?]ÉrSrV~?ï´Z¾E(1?ƒÇèãøó?o,ô-¥†ã?wå>"¢Ø?v<&¦LÐQ?zkuHqS?ï-‡Ïº	s?"ËV®w"?‡À	l{®k?|R_Ø´Š×?ŒÞž"¼Ú?y"Hšû"Þ?ïºQ} <6?~ŸIV·?1d¶RÆ:—?7ú>'²"Ô?€à{Áö?~J'Ø´Ô_?ïù<Oo1š?I°´¹"ð?!7qH¾=?_	
wÌ?FÀü_@Å?H'v/©
!?ïä^K  ?fGžøš°A?WÄÙeìA?SXº'KW?_þjb3?`‡2Þ×jÐ?ï‹í]Ѷ?vç?«"L?{+4!GàÙ?oùÛü‡?~ÞÿâÈ;?lÖU¥¨º?ïö%7êI'?S1tZŸ~?ƒM_?
kS¦Jry?R´g"ž– ?Rç•Ë
Ú>AGN3FGL J1223.0-5622@r¯®]á\§@Š\å´$À9_7T*#ÀÀ;AiÂ;yS?è~Õp_c"@"üÄâ@4Ô@®¥¿ç£Äë¬â¿ç7Ì@\¿ìð³'ÎêοçG¾É1•WUNASNone	?ëÔ•*–y?¼:Aˆ?´Äm€&¥?¸]«¢rÀ™?©5ë®Á`?«—`à8¼?戆[¤?ÐKQ£â?ºޗÙÄ?½…_˜õbv?ÈÔø™ž?ÇÔ;"@?êËøå
?¨àY
w&?¬Å0ȶò?–å§m
?»=¦­íþ:?£}ûïª;`?ÛvpA(?º×‹`öî?Òï!¶^ r?Á|pòd?ÑþÃÓ1žf?·HË×^•?îft|iY?¿ý¹5¸–?Á€".D?£~'ŸÂƒ?¡7ø2äÖD?½­{ŸnÖß?ì&2V"aK?Ɨ0uyæ?¦ViˆÎ¨í?²‰?áðµ?³£8…=Ó0?¼`$(ºoŽ?î2ÿCö?"ð=ç­}ñ?˜y:>¼?ˆÕBi? ¢#ìÄÜ?`«³Äàg?çEqìÑO?«!ŨW?™íß8ž?¦fƒÞð†}?ÀPMÉ9&?¡o(½˜±AGN3FGL J1223.2+1215@qY ¥&•–@Rn•¿ðExÀ:Uÿ'E7BÀ;Ôzª3?âæêÖUÀ/@
^)Òâ:@´ƒàtÊW¿ë¸Kwn¿šº"|È¿ãÆÔ²–¸¿êjx"nëUNASNone?î̀ÈMS? ú'H·WY?¡WŸÙa¡)? 0V`Y¾?n:0æBc?l$ºÅôKƒ?ê«x:"±?ÁXÔÑí·Ã?½þ½_ÇeÛ?»yb_¤3?©K"¬TD?«5ƒOÃFB?ìLa®ï??¥ˆ7?³ÿ^?²a'G§û?¡MPTCœ?¦vÂíåq?'ÿjËÿ1?å)·ÅÓ?·Nj)ìý?ÓDu
›}?·RÚÏa*&?¤ù»½6Õö?˜·Ãç{Ü?ï˜_Uâù?ˆ¦"
ýáÆ?†Üfç£d_?‡/.˵ð?X^íû1?Xs½a&åã?î¼v¶?Ž?¤q[ã°²ô?›ߔ‹Ï? }•.µQ?ŠÖL´Uàò?‹®ëUòým?îyö¬wËF?•†Öû"@_? 9¾4%
?'lÁêޕ(?M®,?|üá—QP?ì'SûæÑí?º½Ó (3?¸yË?{bn?œíç«s¬?‡Ü§¿EI?~d'؛;øAGN3FGL J1223.3+0818@q¢éxÔýô@Q'êžnëpÀ::H=†sLÀ;ËÿwD?áP½R¡Û@
÷Ú·R?ÿÁìžú+«¿å6l³)(¿Ä¨M ‹•¿Îy¨çH¿ë÷4£[ö\UNASNone?î¼ÎVS‹?¤xM'º??¡¥»Œ™½?¢²åv¡N?tjøzZN'?xz97Ê=Ç?é?³MŽ—ø?ÈìË(÷‰Ô?ÄK¸©îë?ÄÈ«#ž"?«óœC'ÝÛ?¯#9g–?넸¢çC?§œ aÄG?º¤T§ˆ?¥5$Jxy?£‰6²#Å?'Ht%%ZV?ê²äAĬ©?µàš÷Š"?¾Ò}{Uá´?´»AÅÁA‰?§,Àé™Ö
?œu"Éԉ?ïfm¬D°Î?"Ï—¾‰NY?GN±'?'-½Ì€?hØH†Å—?p"vßlL?íÁʯÞvæ?²áÍj'<?ª¡¨®JÜ?¯‰y|Gî?"Áf«õUœ?"Gl;—¤°?ìƒ['†?¤E}Ñ{®?¶Z¥õj¡?¢°¡¡d?–1¾R±^Ï?‡òš,_± ?íÃÓÂ	zR?›ßrXòfc?®8ë}îÁŠ?™æáƒSŒ?†'a—q6?{§y¾¡R®AGN3FGL J1225.4-3448@rŽg ù	l@;†ƒ<`À:ºèÊYUÀ;á'o°'¿ô±ó:ß¿@1PÊÈ»›?ü'ºž÷Ò_¿Ö25ÿ¶¯¿É3Yö¸Ðä¿ß­[ÿkl?»}ÙI²ÑyUNASNone?ïóÜ㒮e?JjѓÍæ?>‡ƒBC_9?6.ėèYÏ?P¤X3M­X?En—‡›¸w?ﶸÁۊ³?ƒJ[Mð'?n^mYÛÏ°?wÀÒjàçi?uth…™P?y;BÊ͒ž?îàÔ8¦åˆ?ˆ²B—[$4?Œè¦d[³Ö?~›t[5̑?•q%²=.?ˆÀ­S™?ïͧ' ½?qՈ·6÷?Áꔙh½?"Ô]~^±ù?y$zâ¸?qÄK?Á?ïúkt¦?9lLB›û?)#рïf ?#9æ'˜Œû?@
útúu?5fbno?ïäXVz­h?fgù¾bF?W‡ò*¾ë?Sø$C  ™?_ÍË:!É?`ŒÅmf‰?ïsˆ¶%?v¬ïɑWû?jTÄ¿Ãh?p³½5±7?ƒ…3r&šÀ?jÏ	£yå?ï÷÷_m
?D —Æ-Ä>ó(è:ž	¾>ñɲV»œ¬?O‰=œ¾Ë+?Dxb+ó¥CAGN3FGL J1228.4-0317@r;jžnëp@M‰‹ÖbwÄÀ:ìÝäLEÀ;¯
õ´MÀ£$u«'á@‹ÝËø'@,û GH>¿Ìˆ©'
.,¿á™âGeù¿ßX#¦ô¿åôŽï`d^UNASNone?ïó}µ&VÆ?T˜ºå"T¿?N‡ð•›M?Pçϛ'õþ?C;i%?>
ñHdþ?ïÅb-ؼ€?†I†¼C*?i<[l4¡?w«¿~°ñ?p°»a¦÷C?€hc…ûË?îânpåµ?ÿ飪ç
?•¡3ä*"?ƒ°Qe|b?"«õ–ä?€=шzŽ?ïðœQÄ?qÈ˜¶å>ÆË!Â|…>óÁÿ?¹]¦?_ña¸FúÜ?q&L1?ïübÐôhŒ?5pî
‹æ?.ûø'<?/]%Œ?+Bò­pMK?#:ZoÆ÷?ïêëî"â?fˆÓ‹K?S]"ë¿î ?S߄wÏÙ?Xt'Öá='?`ˆÏºz?ʙ/«?v8Ò ž‹?~Jµµ â–?qg‰·'å?}bdçÉÇò?dþ•Ö³?ïýM|EÜê?LI@´W•->`3mµ>šœnë.R?5"šxîjþ?LI=
5rAGN3FGL J1231.6+4825@`{ԕ*™@Q`þG™À:Ø£š¤À;»‡Ý¯s ¿º'÷‡
¡@WÀ<pž¤@À‰G'¿å&ËEä¿åV c€`–¿ëQšfÜó¿ÛGÎûü[UNASNone?ïè%0*?f$%•»œ?U䍛¥µ?Z蜉ª"?Yù(K~Ó£?YØ×Äåß+?ï"jlt6M?]FýÌfN?xñ0Em€?ƒR¦šÐҞ?|ٙ{öøC?'úií0X?î]4®)ëÙ?•°Éº]Y?—¬Ïˆ<DÂ?‹85ÔŌ?œ¬š­^Ö!?†sªn>|1?îrÀ6ñ2?šœ»g=´"?Óë÷uÇ÷?Œ7ì}¹?¡_¡£zÚ?–]ËÕ?ïø	qÌS´?KƎ7"?9ÕXãÐÜ?>³JG¼&ö?BïmR?A4·|"êš?ïÜR÷|¬?qµÜÒõ¢?`ëh»J¯T?dðù/1íø?b†u?ef·r/6?ïD
÷)í?'«º4ź?ˆpr…Ûç?~E³ôÿ½Û?†ŒÏ¬‡$O?pzږ?ﻀvTgƒ?t3fmH?fyŽ8Œî?Y]²ªŽÖ?w6¬ìˆ?qˆ~q{"ŠAGN3FGL J1231.7-6513@rÍ×süPÀqOøÃÌÀ8Ác¡ À:ôóW{?óñKle@üóʒŠÝ@e#?ö;¿àÐ9zŽÖ6¿å¥+XÚs¿èd1®ßã¿î‹ºù¥)UNASNone?¶!¯Ê@í?±$V3Æà?å´ûÖÁ?ÇnöEÙ?Î:û¶‰?ÅÂóÉՐ?ŒäE
!?—ù<ÎÜ+?àO>í"0?Äa4X!T9?Þzb<ë?Ä솻ñ]P?Ñü‹¸ÁÄ?³é‡ˆ«ýÎ?Ö¿FÛöOA?´¨ÿÂ\JH?×D-kóîû?¸Sœ¶Ùü?Ã(ê›>à?¢m&¼/Û5?ዓêX#?²O•Â!?ÓTÖ6Œ?®	­\Qâ?ÆÛÉP&Å"?½l)µþL?ãDõÁ–@?ÆmlpÓì?Ì.Úø£Y?ÂïIY:Xì?£Ü!ñšÌ?ª£Îîékå?àÀoÅvÙ?½ï|[Cü?Üœ7ˌ?Àiù"3?á¼øéá/°?´6C<
ŠW?ÏAø.5®Ÿ?¬¬îè®ê4?ÉÊ$*E' ?­²sÓ]öÛ?Ó/¬k'f?§ÄDÃ?ßØ)LT—?­w¿Œìh?Ëvö×bR?¡2]Vd"MIXED3FGL J1232.3+1701@qeŒûüeA@S¾7`¿]yÀ:K1"·ºíÀ;·­AJÅ?µR"Ž49,@
» ì^¸r?ýeÀÂ}i?â÷ñó;»1¿Â½¾ßE¤¿Þ}4B@±¿Û¹'¿ÚÃRUNASNone?ïînr¤bJ?VQfêb¼e?BGny3"?=åá1lÁ?Yÿ'_
R?R|³¡Vù?ïO¿k˜Ýæ?Ÿâ‰QÎÇ?€&=\¦üÞ?8<ÿ²Ã?‹éç³Ú—Ï?™ãÔ/ªƒ?îì^D{Q|?‹rœãL¬[?‰HiŽ)	?x@ƒvï*?•Ð¢¡Éø?†U››…	È?îP¼?œEd_d?–½°'ÇΔ?ÜÓL?£ßV‹Sºû?—a8l<›?ïùs¯'›?CÎ$ÃAæí?,:²‡<üá?&ÀWßØ?C""ÐۋV?@—AKzoQ?ïƜðÍCP?…åã˜B
ú?e ¼i '?m¬Å¾a4X?qð·#Ìo¦?ƒBӃ-'?ïy÷Sø¿^?}Ë('ÝF?{i@ô,†H?j«}`ïª?ƒÍŠ{[M~?xâyé6à?ï‹L…¥×ý?y9vùÆ|ê?y†WË؀ì?eDo3Õª?€i²´
\a?tՇpÛcAGN3FGL J1232.5-3720@r¬r䎊r@9`œä§´åÀ:Eä9ÐÜÀ;Ã3{W3¿ËÝ«Pj‹@#
%­c¦?þ˝_¡Ñ!¿ì¾WýJ¡—¿ÍpºZâØ0¿Ù2҇™3e¿Ô"•ziíHUNASNone?ïüÕÙeâ]?/Œ=vâdy?'%uÕà§q?"oÒîsip?+|ö[Hž}?#w§eŽìï?ï¬$tJø?…ìýÔ2šþ?pþ®¡´ŠR?xòn_¨?xÿ?A²?±è×W²Ê?ïcHo-4?~'SÔ°Gc?O¬ü#Ý?uøŠhÖÏ?…ÞM[[#?qCìá6³"?ï¦Z漞=?xÔñ9`Å?FÜÈxÇV?GÿÈ*YM'?"ûyÂëuÐ?wͦº]H?ïþ'±˜
p?]˦¾r¢?qz¢?¬;ùÁ?8RýX´(?
õoï
/æ?ïáíež•W?hNX	w¿'?Y¶ŧ?Sø³I\Ú?a"?ƒcM]?b߯™[i\?ï«æ_'Y+?oÙ¯Yp=?sÞµâ‰?hWSkßµ?v.¶_Ü?a±nxáĨ?ïíØÏJ¼£?Røþ¬Ša?4£¢¦N+?'[Í¿\ã?_%xé­y'?PÀôï†ÛAGN3FGL J1232.8+1332@qÅ)ûçl‹@RîÐ=š•BÀ9þ©1½nÀ;'ÆÞOâ?֕YscÏÞ@o÷oF@]o€–hb¿ç{YŶy¿äœo
éÓ¿é{€cŠ
}¿ïþ2£nQUNASNone?ï¼vľœš?}mZ}¥?|\XS§¿œ?{
âÑ!ï_?U¡m´?R/ϔ'õ—?íE³%ƒÈ?³Üv?ôj?ª¸¡ûö'"?­sX@¢¡D? ì-±±@ê?¤œÁáõ"?ìÈ×(¶E?¡Ñ‡6#?¯©àé®<»?šÆi ù÷?£È¬"Žÿ?'lú%§X?å‹flëI?¶vß¹Ç3?ÎRÀʾˆD?¶á‡ÙxÎ?¶ÿK
}=¯?¤e@ ¬rå?ïÚ©à^D?qò'—w.?o»žÔzkÛ?pøùu,?FjÇS¸<?B£º­Ex?ï?ÙWRTê?›$»Ã‡v?*©ôéH?•k
¤™ˆð?'ß–|Nr8?…š¹éÁa?îxÚNëu"?'jÎ0ù<Ú? uøáö?‹Ék%åX?«Ê5Ó'ƒ?㐨qž?ì迆%3?˜¾äw{q?±Ê–
\¿
?–KöÄ/(é?›½·h]s?ˆêýB("AGN3FGL J1234.7-0437@rqe"¯O@LÿŠC»@³À:ŠE{4SÅÀ;³"¢Ù´?Ùôÿ­@êI5Ó÷c?úb¿?›vi¿ïÕ@–?"b?åÝÝ*_qw¿ìõêÚBÅç?è\k˜ÕN|UNASNone?ïØ2a"²à?z–®Oژó?r–¯¿€Êõ?zRSîïSa?5øŽûàÌ?7ª, ÃÓ?ï¾O¼*é
?ƒ­½JËA?mô°€Çe?z½>üüÄ?qÝɉHV?uc"Œ'òq?îŸà$dۙ?"ј}9?˜]s»ž2?âpho?"¦‡¾¥Â?"º8©w
?ïÀ8R4‰?†+UÍfü?e™|=J\?€4ijóÀ?ss%ÊëzP?{¥xÇtÆ?ïô¯ú.?a
¿*´Ü?S‰—s?`)~E)¦ª?1àS?éD?2.cvîæ?ïè—çV«?eÎHz¨Ÿ¿?UÔ>%í‰ã?VÀ˜'\?Z'1àÀ§?]a+™2Ú?ï2JNž?‹6Pˆ©ha?Ž…9ÂÜ?‡fgkˆµ?…fçDçƒ?yI%X}
?ïøñȧ®?U,"ö§´?.äѱ•˜?BU"Ώ?D¨à¥«Š?Q¡'èÑ·AGN3FGL J1236.5-6154@rÒЛùÆ*?íSó.ZÀ93»ËóˆùÀ:Ÿlç‰çu?ȐÝ,Y›@Ø+Ú#w@ð¸`Y1¿è­ˆÖËÆ¿ã-\òÓô¿é½)Æo\ü¿áI踪oÄUNASNone?çñêµãI?Ã¥)6@j?¸°%Ë@±?¸Gtj­jS?Åp*ÂB҅?¿™úû^[?űg™T?ÌBÍÔx‹?¯îý#VÇ7?¦úç~ž?蔶M"m8?ÌtP'á?âqKl?¹÷ÉÙ0?þ¯Ã¬?°ELMQ?Ñ>Ý‡§v?³ ú'Öýj?äþ
q­—R?¿Å^Ñ>?É /'?‰áÿ¹Ø?Õœ†!Üc?¿:ûOR^Ù?í$·_Û»[?¶ú¥å¤¬j?¢²>!¤?¨[퀋&?«ìø½ö®?¯¿Lzº´?ѧ¦Œ
(½?Ô{ˆ)¸=Ò?²R—hY37?©ÍYë|çç?äáÙÍ‹?Ó"ޏ z?éê&è¹Q?®Dœèޚ7?³¶Çu÷ˆ?¢¬˜Ç.Ä?½ôJn?¥Ó™V¿ª?êO>qÊ?­xÚ%]¯?‡1z÷ò˜?u¯Äž>Î?ÅOwÙ?¬–+ôý!çMIXED3FGL J1236.6-7050@rÛMžƒä&À *™0¾À9Ôÿ¢³õÀ;dÎ#"¿îÎ2c»¢i@ß	»?²@©c `Ș?íM³ØØ¿ä##À›Þe¿ærQ2;€N¿ÝÒ"…¶¹UNASNone?ï'|¡ç?…šÐ˜Œ½ä?dC§iOH?cö¦¢…[?†P^n¯½?ƒP¿ø]?í†pUH?¹¬PýÝk?ˆMÚBE
À?0`ÌǺ?°ÂÂDç_?·m·â†¨?íÉ.3ð?˜üa›î‹ù?@fwƒDC?Œ<ª«9Õ?¤ÏK7Þ?'2]èÃ?íÞ»Ôݬ?¢ÿxõÎèu?Z—7{)µ?_â£ÃP?°¡©Z)¸?¢Ö¡¦'?ïÛ0¾õÛ?lé÷Ÿß?S—:æ¦'Ë?R…—"‹áÁ?k1¤{Á‹?g"Gæ?¯Ù?ï3LJÜG>?¡5\Ýjm¡?r_¹JMNè?u¹ùbæU?"þˆS¡?žYpj¾hE?ï0]ó?†¶ÜLPù]?ŒõÀ®Rے?€\°5¹‰?Œ>(Œï®?z/æPm2?ï'×î
†?€'Ã
ö« ?3ø¢#ž'?-ØÛ#0ŸK?ŽªCϧar?€}KxƒVAGN3FGL J1239.1-1158@r£6âë@IdÿñÀ9­Öû#ø-À;"ÙHÜ?ñ10N§X@D£JÈP;@ˆ ÀaŠ¿êä¿hìt¿ëäQZ)…ú¿ÞÇ\O≿å'UZPUNASNone?ﶺ¯?ýt#¯,â?vªb-Nô?w›òæš.ç?l¥®Pæòp?l¯ÏU.*ï?î~vˆÙ"?«<e©¦Â?K2?£°†°ˆÉh?",…ý¬ÿØ?šm䋺›¸?ìÄäGVš…?¢îÁ±i-¼?©?GËh5?™
#݈dq?ªrsÀ
)v?—¿t:2­‡?é
³qÝ?¼"Ô'Déó?¾&…÷a‡?¹,T%Áç‰?¸ðɛp݃?®ÇŸX£Ä¼?ïÛã^ÅÄV?l1w0·þ?g™d¼?fŽ'ZµH?Zñ*Ü?Uí'…¥&?ï…0§£Ù ?'nAb\&Ù?õ9Iðƒ?‡IÏE¼¼x?y}9·Üü?€ØFQ?Ý?îbCÕ±'?—†Nöù•?›¥˜h\¯?J÷ÑÜw?˜§'ë)£?‹\ƴ°b?í•Á6°Z?¤þ"žš\?²qÅÿ5ý(?¢L*Ör¡?"f/ښ2?Î°ç8êÊAGN3FGL J1240.3-7149@ràÝDUGÀ!ò7Š°ÈŠÀ9NÅÚjDAÀ;PPKqîZ¿ô4ÏÅЄ<@ÿ÷1Ð1±?ÿo¤?åÉ¿ç3àÃ¥v¿ãü!‡ Y
¿ÛyVÿ§PοÒíƒ~Ø«±UNASNone?ïëTÕÍÚò?]qÖÈt?0¢ô5»~·?)îl°8f‰?b–ËÝÞGì?[ä:Ô¥«?naÔÔ?«'2fíem?|p鱙q?†rn4ü?¡æ™<ãœ?¨4¥-³?ï%Z½TU?"Nÿ—"d?'"Ó$Yðo?sՍ‡²Ò?'>Æå,??~ǔüXg?³=ôF?~ۇe½†¢? M{	oï?
YÂzŒˆ	?Œº2Õæ#?~ÏNžQñÜ?ïôÆo ÛS?LÇÏõŒ¹?3Àí
²V?+Ðy®{£ê?Qƒ;<"|?I5,_'?ï…xìÔ?•Œ
¬p?fÙ%>^¥Ÿ?m²ˆypå1?ˆë¶s¤Oq?'ºð&O<W?ï¥q3ýf%?pØéÒHb?qÜ᎙?^ßÐh¬6?{j"\¶YW?gÿíp¼AÃ?ï抷î2<?V·¼nÌ>ò{½·D>ë‡iøS0Ï?iQ%	˜eØ?V«èÈI9AGN3FGL J1244.2-6227@rá˜ÜÛ7Ê?ÚbÅGtÀ8¹+0/sÀ:~"Ž½ž?ñZ:MƒÁ@
°(ù°@—kˆ±j?ïþßZ)Rp¿ã6âƒ~‹\¿ædæo=Ù¿ì¬wJlé@UNASNone?cÐáÿkßè?d• ž3T?âžWáé>?Ðùk'H'?ڛ®x4*e?Ðb—Ï¿ñ?ou1{OZ?ŒLCLs?Óº'¹>‹½?ÃG׌Õw?æIrSžQ?ÜH;";ó?¹C.,RN?¢SÏûtbÐ?ÜË þÎãº?¶Ú~Lr[?Üã"všs?µÎcÃÒZß?±ÒoÑñ+?¡V>¾ì4R?Ùeѽľƒ?¿¾«"÷Q
?áÉ&¶3i?À–1åx?x)«ÅÍ€?O »o¬ß?âNl¨'…?Ï/Rq¦M?ڜ¼wʚ?Ï5ÑÍ:Ë?…{×Ó?™
{Næÿ?×Ùd`ãÖ»?À&Tašéj?ã¿¿1®¤?Á"qz|Ú?Ðü¡è·?°}¹}F:?ÙÍÉB?±ä=
[ñ?Õ6rՁô"?³51UC›?À¨¶¶©®?©iΐF^´?×æNmÝ?¶&­é²¶¡?àK_J®F?·;vÑ'+fMIXED3FGL J1244.3-5515@rޗö+jè@gB™ØƒºÀ9_ýŠÚ¹õÀ;O¦¢–˜]¿µ\)^ŽÄ@«wÈ8"o@õò`L–¿âX´^ìÊn¿çt|')ð¿êŠ'=:%É¿âE&M¼ŸUNASNone?ï(ªñ'A…?–ãýO}j?ƒqw…(c˜?ƒ–ì°2Þ]?'1æ£%"?'Z¾UÛ?ì#®¨@ó³?Âs¢¹þ¾â?–ý›Ææ? ²‹Áx™?¹#EV˜µe?¿Cª=š"?짱–ª?É?¢É1€¹Jz?¢6ØZÿ½Ö?Ž*íMý*?±§À/O?œÒíu"?êšK›½hß?ªHü‹:âþ?™o±T%?":$ ­Ý?ÂhÛeÖB?©â—øZ?ï˯	(®Ü?vb[=ã?cñ(ê=w?c«+¦ò©?p/󻶓g?pzù÷\?îñ×LäD?¨'…°°?€i°;Õ?Î?‰àü`Œ}i?™>e¼('?£C÷óy5?îç//~®î?†êÂÌ
¢?Žœnª…?{t»VîO?"Ëⷲþ?}«¸&ë?î7ÇÜ;ï?‹qȕ»?|V!/´¨[?h\±¹?£¿YÝò?Š*¢ÐUì'AGN3FGL J1249.1-2808@rå2a|Ú@A\ÚãæÄÆÀ9Ý68¡1>À;ªíñ	Â÷¿ç•ÿø€§@E
6ÊA'@ˆ‹`pÙ¿èÛÃoMb+¿ß)ŸÑ`I¿Ýj…ÿLÀ'¿ÞŽk›¸
UNASNone?ïò{Àj¾»?SíöÔbaW?@Å͚&?:{'øCCk?R¥˜n4Ñ?O'–ñ€"?玲ølõ?‡¯æ@?r3>'	?x|¦óÈ-?zv;fúˆ6?ˆêÒø²?ïZXAñ	?T¿7}¸?}ӟ¤s…ê?lå{Ú!?Š€/;vú?x>(‡r§?ïlš"µÕ?'Õïø?M<i0#íô?HþK'ME?''Ú‡€?€°[3ΪÆ?ïüÉo¨¸?67ðÓ$Þ?'X]!M•? Î	¥²iÄ?3í«WêíS?0›R}I=.?ïàlי¯i?hA½P_>V?Zµu½¦O?Sd?U7^?b8m'WX?cF°]ºÍ?ﭏCÄÚ?lP]QF?qD[¤îmÑ?]À9,ý¨?wôF´î?f/9dÞ?ïâY¯ës?[}­e¸pf?3RœZŽl?$"ÓŸç—?k<¨þ¡b?ZŲÀöćAGN3FGL J1249.5-0546@ràë…¸R@L‹fÉûÀ9óÔCédÀ;mQ¿tè¿àAg©\…<@³g€Â³@M¤`r¬?ïEcòmÆ,¿íc\›·¿ÀÁÁ‰¿è¥åÊʔ
UNASNone?ïíЄf?a¾Œ/µ7¢?MBû¸R®W?RBQ'Ÿµ?U½x悕Æ?Y»w?öK?ï¤â´¯ct?…ÔiŸŠ?t€'µuY?zÞ«†}öb?yâ
Ħ?}u+ÛÜX?îQo*î&?•6Žšô?u#a'¼í?ƒ—ÖiUë?¢®~<¼(?'"ÖªØA†?íÿ#€QÖ?¨ShÍ*?gd½^þ;?pœ±x?®—| …@?§éÄ=&ê	?ïù€~.rô?GÂr"{R?8#ºÜd?:öÕ|,?;ِ¬÷8?@4ozWÉ\?ïÝÀöˆe?k'¼Å^<£?_¤«['é?Z1u—?bl³'Ø?c{¶¡‡è?ï5ð<Ñ?ˆ±W=?ƒénU_Ž?zQp8ãÓz?wòP3?";4ð÷?ïJd
Ú?'OæHOS?W="{HÓà?Nڒ¦å"?‰E´"eºÿ?Ëž¸^"AGN3FGL J1250.2-0233@rå'¡ Ï@N'=¯÷¥À:—öÅĚÏÀ;‰Øê2¿Ô!‹ôs
@
5I¯?ñ€y¿ïôÍÁᮩ¿á Í‰¤ó¯?ç³p;Á?êX•íUNASNone?ïàBˆ:̅?v"W RSá?/ôÅOF|é?2Ò2µZz€?m¾++VO?uÔVÏ/«§?ïÄËÄíë?¡M¯k¬?jÍÇ*ÄÍA?xˆ©`ÑÆñ?p39ùVÌ?s?
q;è?î!—tÔÄ?œ8!7:ÝT?žá H©J?–[Ô%×a?=/ߌZ%?'c"AÑå?ïÕ¡á+B?"wò+^Y#>ò(>G«¯Ò?!Ó?Ðl6$?uHÝ3ã4?"xJi…ª¤?ï߂7|?x"jt)Õâ?'­M´aâ?,6jN|È4?oô%}$Z?x|@<6	M?ïé¿Ámëb?d»:KPñj?THa&6N´?SåYϨ?X8i&¼?\&¡·ǐ?횄N	?¤ì)Hù™	?¦Öêßâ?Ÿ¨"ë&W—?Ÿf¿t$?—v«ÜPô?ïú¿'·mÚ?L³‡•Àj©>閖,ÿCV?.õJ\?D¦Í_î?L"¼ sAGN3FGL J1251.0-4943@rîƒùd@*GЍK­}À9ÖBƒ2OÀ;tˆhî?á;­2Ü(é@¹ÈQ½âÏ@=ÍØã\?æ7€y%õw¿Õó(¼6Òz¿ÒÖ"¿{30¿é¡¿+é+ÂUNASNone?íóo)ó2V?«Üx©n¹?ª1ú ?ª·碾?Šçmœl†?ˆ¼Èä½.?äfe–¡†g?ÉÐ+*iú´?ÇߌڐÒ?»tû²'?ƆÜÈÃRÑ?ÃËs³x_Z?ëêH_â‹?¨¥I2{Ï?³;Ûi¶?¤opËü	ª?ªãÃØ^/É?•=Q¿ò;?äº%¢žGv?¸VðLý¶Y?Å£%‹Í?´™-+9ó?ÇtKOùV\?±¶
‡6x?ï_"òC\?'2&5!^š?ŒD)Ò@¼ú?Œ4\£Ðò?w­³"¶Ù?vóܖNw'?ê⛣u?¾ ó.z*­?¶Å'·¶?°(DØ!>¿?²Òbå£×?³T¹`vqÓ?îPȶ×[á?™ªG-1?¡·êÎb?–‰…4~?'x½J¯-?xï/³?ë˜;$¬?¢íñ}¹ÇÀ?·¸7X¸§?›ÕeþyÑ?¯–
øN?˜­¦ÝüãAGN3FGL J1256.1-5703@rùHè§ç@Bæê…DxÀ97¯h¸À;Ð߁w?òùéá½)@weêÀ}´@Š<€c舿æ"ŒéC)¿è-¶G¶^2¿ëûGC,òÊ¿ì/%\…èUNASNone?åW;…èí?Ćè7Èq?ÐkƒˆØxŸ?Ã"
Î?³˜­Ë±˜?®Ú"<>?n?ß·J(1]?ÐFÅÓ©0?Ê1N+²
?ÁÊ¢ÝÝb¿?Ó90¹ž?Èí€v‡ñ¦?ã¾Ü|BEË?µy`÷¹ ?ͤۅæù?°êÄó¼/.?Ãêé3qÜ?¦®nùJ?ÑGœu°Êý?³&·ÚwZU?ܬ^¨Vö²?¾Œ>ÅÁu?Òáø>Q?³Ä¯Pè,?èIáo"ƒ!?ÁU»yÏ`?ÊEÝÚ¼#²?Àÿg©²?¢Jq•Óî(?œþÿ‰it?ççÃ@ºä?ÌñGý"?»FL•"áý?ºRDõf?½̲SWt?Â
eê?¤[?éÀn2k?È?«Ÿ–
Ç[?¿"­"«Ñ³?¥kŒuW?²gàÙD
Ž?š=­Kz?à"º¡…?­úeєR?ÕƉ½¿¤×?¯ŸnQ¹¨z?ÄDœf0>? ùŽŸÕMIXED3FGL J1257.0-6338@røт©"¿è¨À~	ñÀ85«³w'À:‡/	ØÆÖ¿¤8Î@ˆr@ÿqŒ_Ig@ò]Àz"¿ìÞ—ÈšI¿ÂBfÊíØ¿âGŗé¿éY˜ÖëUNASNone?í(³ôŸàÂ?¶Ï>5L? ç<¬Ý?¦¬VÄ3«f?­sÙuåzè?²•]…ž?àšhv‹ø?ÕiÙÂ9Ý?§TùÝu=N?©¼9,ü ?Üä+ô$ª"?ÔK	>Ô7`?㺩3Àw?¶¹ªèšv?½'ɱ9si?§‡kH¹²?ÒeØAJ"8?´Ši˜ÂQ?ëčIîÐG?±$ Þ>[¨?x«(ÌÔ?t÷s—ëY?À(q'ƒ>¨?°ÚxeèR?îõÿèqÝ­?¦)ÓiGz?Žetôª©?–äÀÕ	ìš?'
H€û–? ¼÷ÇÁ-?æ-Y€ ?Ԑ@OÛh?£l}qcÓ6?¥BðÁMܐ?Ñ7½QëÁ@?ҕÀ^Ýä€?éÌkŠ°·?²H¬'ª˜?°²+î´?¡c{x¼í@?ÀuG%" G?¬HqÂ!?íõßü¬?™hÔ]mw?i±—"T3?`ZbiZ ?¯ éŸù?˜àM4yAGN3FGL J1258.4+2123@sî˒:*@Ur\=îxÀ:1—¿¤ÆÀ;'UÙPhÎ?ñ[Õcõ@%ÅäêÑ@&K_yã¿ë¾Î×û¿ïÿÕÝÚ?ïýåu²¿ä§B"èe7UNASNone?îW6¬`Ç?µ,ˆÖ+å?v+"mBÅ?ºÈ4iç?§Ç;ÀP>?´Wœ‹?í¥¦˜±?Ç×—ULj?¡An'ãO¤?»M,rh—?®"7n¨C?Â$XÞØ+ê?ê× yÌcŠ?¬ºÔïß`?«áOwÍÇ?™Ã*lÝp?»RTqØp«?§[ŒV¼?íÀð…0"?½8+«³£?'½>E};)?°CëÉ]?«X‡«…?¸
ו8ó?îè̏»z?°ˆµ7-3'?w·Úøã™Ö?"Qaß}…?œøwS&KL?®2hk¥õ°?햠¼‰ÄÌ?ÅY‹õÊ¥‰?¥_¢ÌIú?¿H!+Úà?¡6֗+J?¸!îærÓA?ìù;¥ë¦?£Ìãþ)¬›?Ÿü¾«A¤Ë?'
üïg?°6ø7'F? z¨Ï­×Þ?ïmÝlñà?ª5÷úF?•Ÿµ¿?¦«7Œh?€fVu&xˆ?'…@"b†AGN3FGL J1259.3-8151@ró¦">jÀ2þRv‰ÊÀ9Ê=|bQ.À;€ü‡7?âã"˜A'@Aà;i@'æÚ¿æäNò_1¿ã-=À!e"¿åSÐÄþø¿ìÁsnUNASNone?ìòÿw«?¼þrŒ9‰¹?¸<
 ?¹Ø!÷n‰?ECôâ"?ŸW±è{ò?éÃ}<h¢?Âáû—)k£?µ–0Û‡?±v©6ÿøG?¼Mæt¶Ò?¼(aħJ˜?êëçù4E?§ýÝæE\?·5;-Ÿ? s%à'2?±k…/
vÕ?˜;Ïã"fÂ?å1¿H]o?¨¬ý<•ØP?•Óff^?£€ëã=|?É.6/x#ä?£×ÐÓ?ù,?îŠ$Ði²?°Ëiáf?žïN¬áJ?¦MŸŒv@?˜>y7w?žÄ`ô_Ù?í캊ÍEe?°x˜N 4?›|V¬xÞ'?˜…K¼"?£v+ú[… ?¨5[¥™âR?kâQ?•¥mRâÒ¨?£Í|¦íà±?'^9ÌH{@?—SÝȼ€?CK™?ë~2/¨Q?"÷¬à£bS?³1¯ZK%?Œ,Rní?°Ü¿'˜^?'"(n39AGN3FGL J1259.5-3231@s™" ä@>Rb˧2ßÀ9Œ‰B37À;p—"6À
eS®þ° @{X³|@¶™ßåƒR¿éÎ]àÓ6k¿çO¶UU᣿çZaµ?¿ïÿ	̀žBUNASNone?ïכ"½ß?r©N﯁?ohe5¹Q?oÃAy˜*'?Qøy­ ?Qãªc[9 ?ï¤9îcJ}?î>SÑ"?r'QuˆÙ0?}ξS28)?{`·B$|\?‡qCèvÇ>?î<Zi-7?—2"t=I? bDÂÍ{'?®ž«ª§Ú?—°)Vz/þ?‡þù02@Ó?ïG‹MF?šnÙ§{¯y?EÚÝÄ¡?bï\!§Z?–_ÅÆë"?š0Ìà¨S?ïêÄþ"Š?bé߯‹ôï?`ë8ûQv?a]ïí¶Ä?AC«2>²À??ÍÞ$Ï÷[?ïàöë·Ò?nlC™3£?YÎíý¶±þ?XDW|M?b!¹âå?fT¯7=î?ïÚ7)É
?Šp˜Ú²±?"[*•wBy?"Ÿõ¿k{?†î§?xÜî¥ò?ï×ÐêúÆk?xî†)~_>òõˆÉ?Š‰Ž8,a?t•'þ>è?xê-²$¥AGN3FGL J1301.5+3333@Z1ûµsë@TÍ+©ÑöÀ9þêUrùÀ;Ö5À¬-?ïôÐp‡õ@'áÂ@-g߸6é¿ØT˜Ñl‰¿áLçee›¡¿è³vH q"¿ïÿÄoAgUNASNone?íîQ×¹?º:üj|Ô?µ5ù×?¸µoð]2§?'ŠÃf<b?'"Ž‰ëݦ?ä¯ÀÓL÷2?Ð'ç^j?ÉɁúÒªÃ?ÆÍ$€½ÕŽ?Ãwz·ùxt?ËÔɐ­6Ú?éºò·Âúf?°fMÖ&Ý?Á7Ñ}‹œ?«YèÝ}?°úž"? àœÙÝ/?à@e|AÖ?»j±úŽ|?ÜÅ	yÑRC?¼¾þ?¥Ñ\q£Žî?žÛ—ã-ƒ¾?íœg›*úf?ÀœÐrk#Ý?«Þ¼>pd?¸+1nk?"¶	üh…?µœpÆÌ«?ëƒ@"9ß?Ã(4qÌ¡?³¹iN²œ?´`‹ÆL9?°,ýˆ-?ç?¾+Á«¨ ?ì|"9¢&ö?¤Þ1Þ{IB?±z›¶Ò?žÆ8³ûš–?¥B,êU?›	Äc—‹?ê¬+Ì%vÌ?¤ªí
!Dˆ?ìÎhØ?£€|±ê8ç?Š(,k"7§?…ÌÀÁs†AGN3FGL J1304.6+1200@s³ …±…@R£öÓ0"À:¬Š7&À;¾òâ
K³?ê$.Eì&@µ[©Éèl@ü[€YV³¿Ö¹®(8Ñ¿â*5è3¿î;²[ü@¿ìÂ[¹ì1UNASNone?ê.ëÐÉ?êfš#?Çoé-;ޏ?Ë씵¦?oÖÉ
š.T?vq|¨Þw?ì%®ïÛßS?¼÷ԚC.?´§;›Fð?·©ç£öfe?¤V™ÊÙçï?§zrÀyé?ê´# Á?¯çêæau?ÂPÏP_¾×?«ØI‡ÒTž?¥1zÍ*ߊ?'¯¦y»}¦?àEHDT?Àm×´\hŒ?Ú쌒—i5?Âx8Üü?¯—Fê0q?¥O oNPø?ìBĘ Ë<?½áß®{Óá?½"	6¬Üº?½Ò×[y¬?hú@«õDn?j¿á…­/Ï?îÞ]1D¬¾?©ôZ&ß_C?—ÛÍú'¨?¥¬X$cŸ}?ˆ±°7û ?ÀLÓñ˜Ú?쥈÷5?¡ésM^ëc?µMˆêí+? $헔þø?–ë0¥X?…Q[µ*ê?ëJd•Uè?¤ËlƒïŠÓ?ÀbG4ÇÞ?¢ÔiI_?"¢Ë$3Ć?ƒàяËAGN3FGL J1306.8-4031@s!° ě¦@6>]ž@ÈGÀ8ñjwmçÀ;ëÃ2X¿ò]kÑ@;®õKq@SL`UÖ ¿æ¤2
$'R¿åðÎ5úÛ¿æ2ÓD
Eÿ¿íHˆ,[UNASNone?ìNÑ|èf?µ/'ìÓ²­?³|4ᘐ?°§gȦ/?¤~s‡èë?¢+ÓQ"ß?í:ë¸90½?½[¾Ñ?©3Pì©!?±ïÅööq?£+)È}?°ü½D l<?è$ˆ¦?®Þ­~`ª¦?Á¾†"jkë?§L""nÙ?»'Ζrêü?¢V!&™±g?êPœ™Âøý?¹bí3ØF>?¨vso{rn?®Ñƒ'Ø°2?ÀŸð¾Í
m?³Þ"jc 6?î¬)`˜é?ª°2Ëú×Ü?¦ß¶ügq?¥ØçƒÏ†O?–¦—Ð?Û5±—Ü
?ï5ð¤w?¥Ï§·'?Š®!è'c
?˜íºÞ+ғ?ˆáîg¿;?˜Ü]²i'?ë90˜	ˆ?¦ißêý2?·t´:M9? Éo #ð?­†t€ˆæ?—"ÊÛ0?îÀmIª?˜L2sõº?pvš(ô4­?vƒ)ˆ—>?¡ïeåaÌ?—;	]¥6VAGN3FGL J1308.7-5738@s4Á¨¬\@jOvÀ9`Ö@†À;"ŠfðÀ^õѨԠ@+[Àðöx@mª_åmØ¿é¡XØçÀÍ¿êöbªÅ¿ãN`5IãÏ¿å'ärʑ£UNASNone	?ìŒÕÿf?º—Ïюþ?'W"$˜›?‡Þ8w,«?¹Ns¶ž»?º=¤óŒK ?ìÀG2;?ÂPEpU0?‹ >½Á?™4?¢­>'?¶‰¾«?À€c>á»?è±-*õ:ï?²h¶Èøƒ"?±ÀªÍXç?¤‡(ˆ_*?ÄZõí¶?«Ç[¨*'²?êµùd¢'?¸#{£¬\?UïŸmj§ï?[ô€uÔ>?Äü<o$®"?¸NÚÿK—?î½íjti?«ž—3§'?sx¿3ýø…?"
ѱÜY?¡²zDÍa?©¸t™ÞM?ï/qÓéû?­Æøáse?r¡"C³žR?ˆÒÊ$¨?•i|ô±èý?©«ì?ík½t®íX?Ÿó'ëKÿ7?ŸoͺªØ©?"<ML߸ª?©ŒAؗ¥0?"ì)Pg?î6¤
¥5?ž
è8­ß?/}Å]E-ˆ?17Ù¥HZ?¬vA'¨?ÿÉ•Â2AGN3FGL J1309.0+0347@sžoü]ö@P'`A‰7LÀ:—10#´:À;ð3PD¼?ðÄð_y@íyj¥@¯i\e¿ãS÷‡û%j¿¹U&œ"À1¿ÑÒÛ
8yT¿ïû|Ë`DUNASNone?ë<™8u½?¾ÜÿàJƒ?Áû
Å"Uã?½µ+¹—;?ŒÀ-\M–ˆ?Š®.u5ž?Ý>ä֝ŸÒ?ÔĀŠKjY?ݛ‡ê`?ӝÉwþ?´–PG)Úü?´.zhô,°?äÙȲ-™?´a³Áf{Û?ÐfE;?éq?²On­¾±Ú?·˜¥…Ž‰k?¡²órS³?å7þP\¨?ÅK­eÜÜB?ÓNK£¨¢\?ő\€«ÙZ?¢
½ày;¦?šQØ1QS&?ë)Ջ"¥c?¾ŸRøí´p?ÁWK…ñ?½)eXc2C?
öO$?6¤¬È"?ã¼³Ú¸rÎ?ÑÝ!Ì·ï?ÔÆésvš;?Ðh†H¦Yh?­ýv½"F?¬Uö2 ?è­^Û‰?­¾tjA.¢?Æj¡Ij0?ª5ïÑä­¢?«"ìTв?—;¹-wvH?ê
žÉ¦Ÿ?²{£õ1'½?Æ°áB´c?²Eeï*í*?'J;äbå°?|Ò&˜QMIXED3FGL J1311.8-6230@sœàuöý?ÑW«ãs,rÀ83¸"0¤À:,[Ðá."¿Ð GÑ®g@©h­¾i³@ªÚÀ«VZ¿ãH4qC0¤¿èðݯte¿ä=`
¬¬¿çõȝNk.UNASNone?Œ$WÚ#ÐÔ?$½‰^R?ÑI iÞ¿?•¢à­8ä¡?ïäWØÙö?Ÿ@
±ûW}?±ó/Çâºò?ºŸÙØ+®7?·‹FÁ®¬=?²Î[—PJ8?êÐ1.²V:?ÂnÝÛ_Y#?Âc½ðø{?©—
¯2`?Ś´R=ˤ?¯tŽ£?Œg?æco2Š8?´uB9oê?ÌÅ£
î;?ÀF6®psä?"vºcÂï?‰:ñƒë{q?è*áe¾©Q?ÀÎnokÀ?ž/CÞ}و? ˜»"Uj?•ª(0ãI?œõÙӞâª?îa4œÙƒÙ?¨aÀå7ý?ŗßú.?Ì!Ö5ùƒ†?»>üê÷°?®#€žÝš?ç(7('¢?Íz3"´&°?Ïæ´r–~?²'±AÀ?Å˯"5_;?­pï<Ÿ~Ç?â"fýØN?´¾y«p9?ÔJ‰®õ?Á»¹¬+?e&Ք¸?|L¾îìs?åe&ˆiF?ÁËj;¦OTHER3FGL J1312.3+8513@^šâ:¸c@?á鞔«À:5-ø`ÏNÀ;ޓ*êU?Ó-}*'èº@
ì¯úÙû_@Œrk­¿èRÔÚs«¿æPÒLàѿ旤ØÿпÑÚÍì\ŠUNASNone?ïߨÆw?pœKÿ 9?S[ô–—?ThԝV2¬?f©?bÄ*õ?mr 	/¬?îâ±Øwd?®§LWƒ?'2[½ƒK?¢Çßoj/Ä?'wi.q÷L?¡uP°K×?íkEøv•?›¢Â±A¶A?™7ƒ‡°ú9?ˆH‹aw?¬¯Þ´¾©˜?—&	FS5,?ëþüÿçΨ?±Jw14·_?§Nz¹?ªüªz±YÑ?´`Ú¥"\¼?§(Fˆ4?ïöŽ¶!ö±?QC…¾€æ¾?9Fðä¤^M?=è0Š)?I!®M§ý¹?JÚî<a¦?ï°=
³žd?'å æçk?sû´%?…¨¹&§L?sæwì"I?'žUÄSì?îö™†Æ¥Ž?‰^*l`˜?ˆaÀå7ý?xÓq÷?"ûî½&Un?"-f(G®«?ï.Ž»Å™?ŒhC®.?ˆh*/ñ?'²Jä)ˆ®?‹ô2ÝÆñÌ?K¹ì:EAGN3FGL J1315.7-0732@s—+Iº@Ki¡lçŠÀ9f'áÇ/ÕÀ;'N+Üýœ¿ú0qÅ?9Ò@"étù&@'JßÍ/ž¿Ìß³={¿ß,Lâx8¿åœVK·u¿Æ·ŽgUNASNone?ïû5s£2?:(â§b"?-õàz'?*rÍÍ(	¨?7\ӈP…Ç?2ÙÈš³•?ïÁÇ 	—¦?ê!á?k]¾§'?x—àH`7?qU9mh?t¶bˆCÜ?ï7õ¶a6¸?ˆÄVk"Œ?‡EåH‹ãb?€§s¦Z½$?Š¼­"–
¡?~¹0œÑ?ïË×­.)'?u‹i›F7]?<JÀ‹Î?4OÅX?yË8hď?u}HN,?ïü­‡×?0Gm=¿í?'É	xȹ?!·–ªÎO?-]ýÃM2?&…u+¢6P?ïé`¹ ˜?e9`¤P›ë?TR|¦þÛ?RûGÔ8?Y Â5w¹©?^`<<Y•"?ïŠã>ºa!?€ûiaPN?Q´îSÄ?x®ÏǍ!®?{vî'ò?t°Ü×á?ï÷:øQ$?LzÔ#
>ࢷêO>àÇ%d
T?Qj°÷Óçk?Ln 'ô%2AGN3FGL J1316.2-6446@s/D')‰À3¼$ÞܚÀ8{¾öJt˜À:Åe˜Tö?à;'1ÈúÛ@¨/t··è@O"/û›¿èeà
éš¿èd€k'ôÄ¿ìÈ`´u½ò¿áÝüó¹©7UNASNone?ïšÚÍҗx?‰c,½PÃ?phÐ%(Là?tÔ+›!I ?äuV_…?"VÆvù†ì?à :l&]§?ÔsYMO?­'mÌÔ\ù?¬}̨çJ?Ü
=mý<4?Ó+Å¥*
Y?é"ϨI_Å?²¿[r?²ygkÿ??¢ä-Œa??À°
¨£çj?«ìÚÞXF…?ê,2Ù¤ª"?¯T´ï(?ŒÛÓ6cã?Š$f¼¢ˆ+?Ł"LÞÞ{?®¤fŽ?Îk?ïßä
ùO¯?lt€øéV_?PÝ©dYÈ?S<;ÊýY?g­j_XûÑ?g֚Qnj?çº2ˆéH.?Ñ'±Ào?¡<ͲB5n? ½±"Ø?ÌÈo"X.?Ïð¦	®C?íT#Lzè?¢ÌëÎO·?œÒ¼'E!?'ÃTtÆ?¬TlîÂò?œÒ±–¥_?íþ'S3·E?"…'ðՃ?xB.ME~?gq·Z¦:ü?­Dÿœ)'?"Ž¯

,áAGN3FGL J1323.2-3901@sZ‡ÝDU@7nhãï(AÀ9ËøÁG^À;q½OH¿ÙõÜûîùG@ŒÖ脎@.Yßð@¿ãÍZÐc–¿èœ±ûÔææ¿ã`C˜õɊ¿éh=2v±UNASNone?ï4o×1h?"AX¿þ•ï?€ð•rÑ*k?'ÚXCíym?ùºaRdÙ?Œfª€‡ÿÝ?î 
ÞÝ<ÿ?¬†^i|L?"Í@h†Q?–¤_Æ94Õ?—1¿8uÎ?¥ðÞ%Äó€?ìÇr|8#¢?¡t€ˆæ?¡Ÿp'#?Œçb¹Ùa"?°ôÝä>†ã?™¶p"è"ä?éÌJÿ,Æ]?©::Ü÷r? ¡³Ã?•|ÿZÆ?ÄÈ떼o‡?§€33a•í?ïÅá'D?€oÿÁ:£7?dðùFEØ?ið'½''?rÿ´Sg?v—Kú=?€ßþ?'³M
OT?y_&‡¥d¢?}lƳsV"?|Ǚ"x•[?Š8ö•¶?îóÓm¿ç?†µšJ&f?Œ«jø'‹¹?{€}<Žu'?"/ÜÑ!§7?|ŠBçñ?î0×Ì&¬?‹ñ®"¹œ*?…Ee¿ìLk?ppÞ}æî?§­Ùf›&?‰}•ÒÆ© AGN3FGL J1325.2-5411@s>¼¾aÏÿ@ ·;dZ¬À9AŒa¢²GÀ; èN2'ú?íñ—Ú;w@¥®¯*z}@Ì€•'¢¿Óÿúܪb¿ä=,°sa¿éX ÌSU¿ïÿÙ14*UNASNone?ÐH÷mèÄX?Å8º{çW?ãB)0X•÷?Ë
K9?Âeldñàò?ÂLÕñŽ£?§ÐzSC?±î&=˜?æX;1s.e?ÆPûû¹tU?ÐUz]
¿n?ņ—> Y?Ù¨$?a?´B§ä°Ð4?ØBþ×6?´¬#€ð?Ì+¥ñÒÑÛ?°wC9è}?´Üó ¬¹? ¥Dþ¤Å¤?橃/AY?¸
2õ$ú?Êí€c4$A?³áõœÝmo?Óë
}ºôf?É,éü]‰?á+@:ân?Í =­_Ÿ"?Ã|鞍}?Ã;qR)?ÁB1;>øí?¼©ý©b?äfݯžÐ?Â(zâ83?Í"XH»Ó?ÀÃÌ;5å?ä¹07Ö0?±Ð!Ï°N?Ðnr;(AŠ?­ú*!?¾8mTÅ]?¢Áxe{â?̉àÀþ?©"±ه¸?✿	ÕÂ?³©_€sKà?Éqªä?¨gP£ñ>MIXED3FGL J1326.2-4651@sQÀ­Ú@/4ƒì‰*·À9ÕÜ@WÀ;0¥:·‹ó¿øÇ6þCè7@
²¨óSÊ-@Ž— <A?ïíȬýj¿ê¿«aB:7¿ïþÍë'MC?ïó
ƒ½²UNASNone?ï0joj5?§2cOf·È?}z.Iàbó?ŠÐËþÔXs?'"3ׇ‹±?¤ç¨ Ê÷?ïPËá"-»?¤É¬Xymô?s«ÄøË4?‰5Q	v»?ûœ`KÙÃ?¡u;ã¨Rç?é³Õ渙?­Z¹`¾™Ÿ?¯ÿ°Óm?›2¾Éë ?Án¨£¼w?©ö°iøhÈ?ï)‰_s®?¢çôœNɟ?M`å­?9¿"WsÛ?š¹– ú]?¢ã•Ä«s¿?ï¦j®¤)?¡×N,Ÿ ?e3ïþK' ?uLýŽ%'?~ˆ
ƒ‹? ˆ5ÈR®g?ïÒY0Èʵ?…`;«²ë?_H}G?{pµi\?n•ÇL?z'‰è:(R?íV	tGûl?ž‡E;ðÝR? F ¹•ß?0Ƈ¾nÉ?ªYHÌ^?˜ÎÈËAy ?ïæî½s¤¤?qÖ§Pð=)>Ä´ògÏÖ>Ü3c¢ê?i,Ïü3?qÕÌuòô÷AGN3FGL J1329.1-0536@sþà"'@LÆ)ñkÀ9ƹ#¢œxÀ;@2芘u¿Õ?Aì@esˆ¸Ë¹@Ð
€CR¿à'Z$—¿ã°q7!C¿ààAƒOw¯¿çt¯œ\¹âUNASNone?ïäĪ-ï?aº Ç{¢3?WBÞ*þë]?V$­-Pc?_4ìæY¦?WIÝgÑTÚ?ïšijIA_?‡½rÈ¿9?v¬Ê°‰;{?{›Òçí‡Q?|€,åÙ?=5Š–?îœbaI'?ƒ³ZPD?ÕÖÀÿT®?f	mÀ¹u?›Ý¼~j?†fvªÌßÒ?íq™`lYù?ŸfØE3¸U?€éÐâ²Ç?s<ò9nç¹?²_wÃ\ÀÞ?ž@èh;ª?ïõ F»?Œ4T)ÿ¬?8äd~éÄÇ?3"jŒRô?L…LJtÏý?Œ6+Fñ?ïÜ/ÎMÜ?l"¥#ÁøG?`D–7Ýb?Zˆ˜¤Øæ+?c‹›˜7ù?e]8J¸J¶?ï'šþ¸F?tÃQ¨Y?z×Þ±Ð>ì?hÍcZx^?'iò˜ô?kùU•(ˆÅ?ïB;	q?~©ÕÌT÷?m¯N›O ?W÷Ï$­îÂ?"µ'Q÷?}fôwÖçAGN3FGL J1330.4+5641@\
gbé@MТ ©XSÀ:dš,fXÀ;øwéE©¿¨Q&#°RQ@OƒNÿl‡@öê?yg ¿å,öŽÖâ¿î–56¿¿±^:íU/¿ä!q)búÌUNASNone?ïûac«K?Gt «.C¨?
•K¤ò:?
½?V×mÂ?@ uA–(á?FǙ`t¼8?ï¦ÚkµŸx?‰Õ¶ˆñ3g?t¸Ðì.l?~®óëñ'?wÙùŸ5'?xnBR0â?îš3œÜço?"àë@?0?'¬žÁ8$x?wÝüM'ž?¡±žÿ¶ü?'ŒìxhæV?ï…ëÜ>?|k'ÒO:?]Àêt>?fîxŸø#*?‹'µTá?`+ª‡?ïümv¥ù¤?Dˁ­f»¦?á‹ÄØö?ñÂ?·øŠ?9˜ån!q?DYª³d5Ã?ïß:›ñƒ?nzðýÔº¬?_/¾ygî?_âÚ;fO?a-…myC?c+³¸UÓ»?ï-çU}?'›ÔÝ<†™?wòÅ5zõb?y|ÊöÒº?–'Áv?''ðdö\?ïêm½P`ž?cGvÏÓ²?P>NÍbv?HCî'&p›?[
F´¢8?_°ÕÔí‹AGN3FGL J1333.8-4417@sn#9Àëî@1í…zþ£ßÀ9žs;`ÿÀ;R`ÊE3¿úœ¤cL*¦@ðwÆO@}þÿú̏¿èj!Ù­l¿ìFÂer ¿Â¹­åoÊ­¿ëÝg:UNASNone?ïæ|y;ð?lO³{ÕÔ×?]•Úöž?_¢Ù¤Åže?V/\Áyk?ciÞ¾+g>?ïw¾ÎQ?–BClGn,?tÉzâ'0?{"ñ¤B?‡«½bÀwQ?"]ħ}Þ?ì¬õ«S?¢Èê–?¦|"x@|Ÿ?•"-C³r®?®´ŒúyÙ5?šæ|ÊïI?îE}uv¤¢?¤…—̕?CÓOÝ)Ü?PgVH/h?«XÛe S"?¤ná!R?ïîŘوÐ?]¦8'
O?TÛƶšr¾?SéÝ¿R‡?K2£7yR?MÖWZ¤¬ö?ïÕ?_ïÝQ?u˜öñ8'?^–~x?XyjXp$ò?k·T˜›0_?rf'.ö–'?îu˜&Á¤"?"e€O€!Í?˜ß`ð²?Šb¶#U).?˜mè‹DË?ŠçÔÙïF¶?ï'çS5Ý?€;2Eä?(FÇ{8<0?)ÅËæ¬Y8?Šå Å®‡?€Ìé'û_AGN3FGL J1334.3-4152@svçl‹C–@4K=áâއÀ:–ßY—KÀ;ºXVk¿ªmyÝ@
4yeqžÔ@

ŸzÚ¿ÃB¿­ªr°¿ïþ¯€ê(Ü?ïè÷·uçR¿ãîüúD³UNASNone?ïå®S¡#?Ö@Œ_»Ò?8$£+Üíà?Kសl×d?gMï5±€?|ë}1í?ïŠ$ée×? m@ .3?u‰¢ÖÜ&¦?|[ä"næ?'±ô=ÛÖ÷?ž¯7ݚƒ?îz…0šÁQ?'p2áâZ>?Š"BZȗl?z</Ži‹ô?¡¶œ`}¬?£ø¼RÎ?îdΜ݋?´
…V¸ë¼?Mœõ4Ó"?pÀÊüa?©<­Â[ßÄ?³ð•Ø›—^?ïãC=3+?¦!¬ٓ?@§Ãb?y,‡?øZ?h'ý(£Lø?£2Ȏ«}?ïÓkú\?{M4±Ð"?c%JžQÕ?e,öY–Oß?io£–
™)?tÂÈûӓÅ?ï3»òg™ ?†¤=À ?|ðö"£o?kBNàÓ\?'Lw"ç&?"ÑP,LÀ÷?ïµkÀ©?ˆ;Ȼ¥?Qä×Xâ‡Y?lí!²&‹4?€htónåw?…Þ'¥üÍAGN3FGL J1335.1-5655@sNSŽóMj@Ã֞ݦ9À9ŠÙã5ÅÀ:þIc `É?á¿0rþ>@Å0Pª½X@´8àœ7"¿ßî·§»_+¿åÚä_ð¿ÝQùX,M¿íö‹ÅùýeUNASNone?é©üjk¦?Ã"ÒÊé?²c²Üîî?±¸5ð_ ?À&5Kݑ?¿s-ìnË?è;L(Äç?ÇØçžp?ªB*P{R?¥ä t¶(?ȂDÕêO6?ÄPv.-)?æV2;Ö4?¶Ç7á%›Ü?½›¶÷šÎ?¦6jP¹}?È!õ["ÙÊ?³07Í?æÆΐ=Ç®?±©¢}ÓFb?©¿T+./?œ^fÙ!·?Îtð¼Yüº?°O©¶à5ç?í¶<•»R?±z-SuI?š­(ÊqÔ?˜¢äI˞?§E¢˜
*õ?¬ò"H!?ìöª0À',?¶h:X%+?šqXs];?—Ú'>ÀÖ?±®Xr¦ÉU?±óy3ów†?êюWKÛ?­C@g;]?±º‰à^½?ä1't;y?·¹ˆA?€í?¦§žKýPð?ëœîK³ÃÎ?œH°aËæ¸?¥I¨vžpX?ŒÉÝä_+?¸s¹hÊwf?—*RÜ=OŽAGN3FGL J1335.2-4056@s|quŽ@5.©÷µ®£À9R%cf×¥À;Ov©ªˆÕ?ÉAy"÷@]EÀÔq@p[­Š<¿çÙ|Oa¿é㼊àCL¿å艧ÝÞ¿ÛnÝzUNASNone?ïò°zléÉ?S/­]>÷?H;šŠ"Üi?H/''!×?M|E(@\?Fà›e^×?ïOÿô0WÐ? ÿ&Ó]Èy?k¸ø¾,?‡/aè3wÕ?Š"J×Ä?›7  â?îCß®¯^?•Ñæëp¡µ?"cì$6Ù?"NÌr³?¡SC?E?ëîªA u…?¥9
±¶{:?Œ•)U5|ê?ˆÎÐÏ?¼øËç°º?¤ŒÔßØ?ïútm??+BAñ}?6x?U¬ìÒ?4ªxqÁªÈ?5äQl0,t?1;`	~?ïÃçðX†ï?ƒ,b~ŽG?itWøZáJ?m·*®V?qQÛ¶'ØC?|³#ÈÏï™?ï]G/ƒ?)?~‹e–3:ñ?'«kb«o?qùcevm˜?†›ˆ²¼U?s´åôÒU?îõO^RÝ?…Ø£Î.?v示˜ƒ?eìZhw©Ø?›œ+ÇDð?ƒ¥ûP
¡ŽAGN3FGL J1342.4-6904@s7ÃAž0À›s¢¡À9§vÖöò:À; ãœòên¿ìÃ4ø@È-*Ûv@8¬Ë¿æöfÏþõ¿êô³|>¿ÚËàiÈ×±¿çج˜5&ºUNASNone?îbwI'«?§¢JQð?n6l=¥±?rSjHè¸ü?§õòÛßw?§8L-È>?êzèÜwå•?ÇöIó¾ÿ?žé+¤´Û?£raáæGD?ÂS¿g*þÔ?Äóoف¼?êïυ'¶l?©ëCå³?¤:>Ší=â?'¦§1'?¾ddoƯ?¦(Ÿì¥øP?éOàýJ1ì?¶|!þF[H?qü™™È¬??l‰›ªÕ?Ê0—?ªÃk?¶h@Û7TÈ?ïRª0Y}ä?•!.)Ý>Í?eñÝ
±+«?n>Nž¹^?'ì~Uá×ù?"¨f™à?îe⃠?°Ü©±?…»õæ«Ù?î[h4?¤1(Ï©Œ[?ªw:°;WÖ?îmΡR"?'‰JÐë?òŞŸÐ?Øàk
)?¡&d'[p†?Œ	µß–:?힠èK?œ×لææ?d"Œš—@Z?U"J–±?²fÔZSÁE?œb
"·TAGN3FGL J1345.1+1949@}Èû†ô{@RìÉ.À:?|èˆêöÀ;Ïòü~¹¿Ø†
á/…@mìðƒ¶@Ò.@Z80¿é…U;¿æa3æÙµ¶¿à¨'v'È¿åìb?vs¶UNASNone?ïözüܛ2?T%* ò?*b?¹¨Þ[?&Ðôzö©
?O{}°c‡Ã?R½Îyïˆû?ïŽ]!7*?‹–'+Èn?xúÿFèã×?€k›lË	õ?Öw»	k8?ù©p']?îÂ
Œc-Õ?Ž9jp?‰Îòq#Ð?vÈâdÆ¢?šÖÕ7 r?†›ú->bÍ?ï…ÁAö'?
{¼Ú~v?záÛC\r?píÚ<
Ã	?—VÑHE?‰æ:ŠH?ïý
"zî*?3dïï|aÐ?÷"¢iÅ?"ÿ.œW?1­v¹!v¬?1Iz›ä?ïÚÎþÙº?p?òº^í?aöÅç>?a'¯œœ¢?d*ï]žN?e³wH±T?ï'óΪƒ³?tx| ‡òð?w™L/—?`G)Â$Š?ƒvf?ûD¼?pdIÅ_´à?ïÐ@2±>b?fŽ]·$sÅ?`&†¢–?Jj›7՝?o™
ö!³›?cÇûZÑAGN3FGL J1346.2-2608@sà)~+V@A'Ó"vóÀ9êwXüñXÀ;³$™<|ˆ?è6'Ú!@‹£š#';@›'`—¿ä•ë8âí¿âÖ^¯§è¿ãR]ƒG¿ìÂ,G(*
UNASNone?ì$ëÀ¿¥?²³TJb+?¹zÆu¾Ê¶?±cùÚw?•wn
´$‰?"}ðdº;f?é
¦ÞÀY?À,lo"ãQ?ÃÖH3þè±?º™ÕöäoÎ?¯üqHJO7?¯J¥µn§Í?ë6Kkª?¨c–Ó?[?·ßóÚ¨Žœ?¢¨xÞÒ͇?¬Ûf˜Z+?—E?<egâ?äÂ;~Ü?²-$fÁÊ?Ï[ãÒ¼•?±u!' ‹"?»84"ò?¢v!—Ü?î¼9í•!î?ž<²Áb¼?ž°‡I?˜Üa@'?ƒ'aœg&B?…e>@kÁ?íäB¯I{–?¨
˚y'?¦©1+
±?£zIúÎQ'?–%G»•×?–²ۃºX?íÀ´ö±?™Ñ"ší?§Ö¨ú§ÔÚ?"_B°©«‹?˜Owqž0?…EL·Ôó+?ë~œ6VK?™ãмžëä?¼A0?)?–(`\¼7Œ?Ÿ'­^–?ˆ!{ì-¼ÜAGN3FGL J1348.5-7150@s6t¼j~úÀ"î%¦'¶(À9¼ÚH¶RÀ;ZÐW›È?ÚÉN[5cm@@&=+""@€¥+ô¿èWt4¿êÉiñ5aâ¿Îž.bج¿æêÜØ2±ƒUNASNone?ïÖs&	ÌT?sx®åø—'?D{Ý@?CÈAÊMc?rC™Yn5‡?r\-q$?ëÓu b²?ÄØ ²ê?˜œaÀ§?¢³ÄË.&?»aPgv†Å?Á6y±U??îã²
ü?—›ÝD'òï?'Annav?ƒÆ»¼?§A&1@`?"§5ɨ?íFbÍT²?§YýžèB?wEfS'ü?zanÆ{þ?´Zæ‡\Jò?¦nçEGR'?ïéßý"¢d?t0¶¯ëœÇ?84qD³«?5ѕC@u?c¼?­0M?sÖl
ý£q?î˜ýoî?³óS¬÷Ü?'‹'0 Ý?üŠ I6?¡ÍDwñV¯?¯ê¶œÓ˜•?ïQ›€Fæ?'‰Hà6ì?{ƒ‹ýÝ
'?hQ}áV@"?×Yýÿ"?€5¤^e_?ï2ŒÉk]5?‡;ƒ…W¯?wß>eR¬?h\Üޕ‡ž?"¶—3ìIG?"ÉÌÅɁAGN3FGL J1348.5-5833@sezÁҝÇ@ß°&£Ø¸À8ô´JÀ:æ$óÅ?´¾ÛÚ.@âøc!@XKŸ©†¿êL:­>ÖÄ¿êYãñ#ǿ׆£˜ÞÖ¿ê¤{X™}UNASNone	?íc]áW"?´]ÎG P?''ôùU…²?'#y¬¿;??°€"¸Áîq?²Ý÷iøh?ç'ÄNŠ7ã?ÍçûJþDÙ?¨(ef›Ž?¨<ïíµ»é?˪ÕmҍÎ?ʀ"gä?â˜9«%â?ºYü–m?¼C㢯Ëh?£ªÊ's?Ó¾"Á	ía?¸©½Y£p™?ä<´fØë?¾…m\¥?›9íefˆ?'Ç"þçQ?ÕÒø[­"?¾DÉfC‰u?î".9	?©SfÇnÅÚ?~ñEY¨Ì=?RŒÛîB[?¢ÞóÁ³]?§'‹ñÛ?íB<é?º¾ØÏ->?";¡=hEƒ?˜äNžž'%?°ß0g"òm?µ¾‹ù:?ê¼É6À0‡?¬V¡zÎ"C?¬–™<°5?˜Ïírò`?»Îi«¦r¬?¦×…"ܶ?êWx¿PÚ°?­ŠöŒ»o?—.Š9ÑÉ;?'8ñ­¾©ó?üKº‡Ù?«óS'ÿ@AGN3FGL J1351.1-2743@sì^_0çÿ@@§T!ÀD(À:¿¦¥òÀ;šCV–势öÀ)æ®JV@!¯B"dY@c cbP¿ÞI]褪ֿì?ž8dË\¿äóC¶……¿¹~"d%EUNASNone?ï÷Rf&¬?NSïkØk_?1 Eo
<D?0v#ñ¸"ú?J&Dê$b?Jž¨ŽU™4?︸Yçì¨?'Û9˜nH¢?mÌ-ׇóu?w»±‰‰Ýã?t½¼'$êk?wíµçäCw?òÌÌÞ?ô8ÌzA?‹a悉f?}æ´¥œ°È?œ\Ža²@'?‡Ìà\»[¥?ï¥ZÈMŒ%?~ "ú¬?:'‹#^Ú?ÉË°}"?††Ù¥,²¬?~LŽ|?ïüšÔÆÛ
?6›]žÎÓT?ƒg+	?EÃàõŽ?3H'¤Ýܖ?3?ŠLå¿?ïäÂízí1?f"ö7Ao=?Wa™~êâO?S–¼®ÀG?_‹(Eü?`¹ô­7ml?ïm@Esb?~j^õ?zûi1¼Ð?mõÂ~†
?‡2:X?xØ({ÄN?ïñéüªØS?P':ʉ*>ìÆÍ
ç!>èÜ{.µ 9?[òz¨µß?PµopͳØAGN3FGL J1351.8-1524@t;Ýcˆe•@FZ³R¨À:E{°z†¯À;•
ùXF¿ËùÈä
4@Ğ×F"y@4`JmŒ¿ì¬ €Ò[¿ãçäeI¿â`ÇúfIF¿ÕùÅÈexÄUNASNone?ïùÕ«1‹W?@JÎNAµ??8Ca–Ç?3å9BÝ :?9E¯…ú?4½¸Œ?ï¬NÎ!ê?ŒƒoýÈ©?sR`
"?‡ÅVÇô3?v†̽,ü?zâ^%š"S?îà€0<î?‹O‡6FŒL?Š¹Aê+
'?zÕÁÈÙ?–"XüŠC?'Ñ—ûÊgH?ïNoÇÒ×?†oÌٜ?Uþ·à¿c|?W÷5ÝÛ³ˆ?"ÝF‹cí?……MÑ&ö$?ïýÖ‡%'?$:Ž§\x?!•Ù‡Ë?g2°>˜?!	ó"B?7óºz?ï㔈sè–?g"_:œ?YºàÆfÇ®?VjMŒ ?_ÐÌB?`ÒÝo ¹?ïŽÿmš‰?s3Íu'?xI"Ø;EÉ?l)['{®Ô?€b5š
Â?f"°_ýF?ïÜM['˜ö?``'áZd?B >j¤æ?6–5ï's?o/ò*ߐ?^?SÝAGN3FGL J1400.2-2413@t&©Ür\>@BÖ¡aä÷À9ÞvlmçdÀ;¤ñ-À?ó¨›C@U;ÉÇ_@@Óàx"¿åÞ÷*T£'¿Ñ²Å1u¿äÈò¯3<¿ïÿúÐÚè2UNASNone?Ý·AçWÒ?Ó¾bžýÿ?à
¥´@J.?ÓÌÅÁüËS?¡›•¸ÐŒ?­'–ÜuÃC?Ïe–aŠŠ?ÇBe³Á—?ä¼`Úúü¥?ÊM?è'?»QÌïeÇ?·"t^'´~?Û4'Fœ¥?·C¨‹Ï×n?Ü"vŸØ?¸™ŒûÈÛ?Á‡²†¥v?¨Zûƒý'?Ô¯âê#'€?µ—/Ÿ|rò?ãWY
æÁ?¸¾ŽEÆþ?±5¹ÒQv?ŸÕ²'Ã|?ä9ÒÛÛ?ԃìBLÅo?ÖnŠ7ã~?Ô-çñãª?'åz‡tlÓ?©¯1§àÐ?àIeÜu-Ì?Ç]RÇß8p?ÚL&çú?Ʊg¥šr¡?´" ~´<½?­Ë
˜ÉàÀ?ãÌà¨÷°{?³ëƒx?ÒtêžB²?²¯äë™Ä÷?·ÅRUÉq_?¢ªw˜c?ãoÌt?ön?¬VߙYã?×¢7¢Ù‰?­GLÙm1@? 'YhÕ?R"zàkÇMIXED3FGL J1402.7-3240@sþ=ÈK@;ØÃÁ‹P+À:-bŒ½EÀ;´ê8v¿×wò.J@Ìdȵ@‹\@r¶×¿å*±Pg¿ç`ƒ<ØE¿é7ÞS¿âçƒ(áUNASNone?ïé1Ͷ	o?b¢>}Ž?JëÅÚ}"©?M²¾ ŠN?`@—ÔV\?\à#}ä|?ïyø\¶o?•ZÜxé?{ŽGŽ©(?'?¥ÃÜ«Ã?ƒºÅg'®?ƒ…s+w¦?î«üðÖí7?ÇåÝ??…?ð¦?{í™Ó%®r?š½Áþ"ìO?ƒûO¾O?îŽ;›ÑF?"-'rS"?y¬4Wɶ?s`"<¡¯/?£ú¾rö?"O,c?ïù5[+ŸÁ?D-'Þݗ?3d°x§?3·óؒ¾'?A áa¹0?=Ý%*ÕË?ïÓµ?$Í?u©yPô‹?cúzu3(?a/´ƒq?i;ÆVÈX?p§LN$Â?ïr"Ùæ]9?t'˜ÁÉä?Nÿ5}?gßéNS›A?ƒ·Iñ!S)?huýëí?ï¸+ô‹¾Ì?pŽ^=%7?XÖHëkP?FÿïYÏØP?}´s'©{?o¶æ¦AGN3FGL J1403.1+1304@vH'ýuâ@Q—á2µ_À:Ájî‹À;ïQ{×?éüQ·Øžè@ÄîÕÒ°@ +ßVè¿äÏì‡cr¿Û4¸#G'Ë¿è|&x¿ïÿ"¢[VŠUNASNone?î^BLù?«ò–»?¨STPdF|?©ÎÏp?ˆ¬W&üoÝ?,¼†	˜%?æ»&)½ò?É=¦9÷.?̕7ïu%?ÅસƒrC?°ü^ÐcèÚ?°è7õ*]?ècZ±9Ò?±Ý3¬$Ÿ?Æêðh!@[?¯­l$	'\?®œ¶/r?™÷"Í}?àá­j˜?»'d Wgµ?Û|I%§ž.?¼Ï™"~;?¦
‹ù…Øì?šOÂ6Ñ
e?×&?§t}‹§Ó? `9ýV÷@?¥‡­WîQÍ?>$GñÒß?'^Eçàr?íqûRq<?±
œY?­Øl-ɾ…?¬öüC"z~?–½Q˜±?"™Y¶]RI?ë?e›??§|ôn´*?»ï;Œž	?¤ý¾ãÿ9?Ÿ´V^[€?‹×•ü̱Ù?êÁ?^ÿXª?£Ç§ù?ÃKäÁyê?¢òʸJ‰¼?ŠñÜ…»?'¿D&âCAGN3FGL J1404.3-5241@sŸ¬1&é@!4úïõÆÁÀ9²ä¥5¯À;I¼2JÕç?ê­-°Åã­@ޒr@Щ¾€¿é½«û#«¿ÔÍ6ŸNdg¿ì/¤`p¿åL²Æˆ²UNASNone?ë"ñÂz?¼Øû!|…?ÀõS A?»DȾ0Ž?ŠéqõÅý@?¢Â+ÑB'ñ?ì<<æT!.?Â^$ù^¦)? Òª@✎?§å-\R½ò?µ´Ã¯iÄ?¼=בvà\?ìB¥ WÛ¬?£Zp7@K.?°,yÄ\ÓÐ?› QáÍy–?«|ºv ¢?–zXVp^"?ç?¡/‡y~?¶΢©§s?Á­ðëé?´ÅõøÀ¸?ÁTfQÌ.?«²ƒÅMй?îÐêÄj?¶q±ôä?™ÚŠ2p?¢šËBÀ?ˆD± N'?´òÑ|s"Ø?ÐEZÜ?°Ûk|ãœ?‹ÍÐÉTÉæ?—4ƒ‡ŒæS?c'ª?™?§Ù¡Áb3Ç?î‹ý·{Vã?"aß}…e%?š¾LòÆk?áR•Ï	¾?"ÁüÏ(?'û…"›‡i?ì­ãô9Uë?œäUï9¢þ?®2y™±Ý×?•p¼‰;[(?¦ïG %'?Ä"ù‹AGN3FGL J1404.7-5844@s…d2‹n@Ki~J‰À9ªÂ©][üÀ:ÍçâÒÉ?І5lQ@
Y»~Ư|@U]ŸÃTS?ï=p?qô©¿ìñ£êƒ¿ãv˜@[ÿ¹Þ'$¸ÏUNASNone?Þb^ƒh?Ði#šŽâ?nÔÜ)ýЉ?l¦–\Ä@R?à°"tÊk?Ðj•‹©'<?â"wüeì™?Õ"N<"?¤,³\ WÝ?¦'‡Cû?Øqy›]¥3?ÓØS"é#?â»^6'jŽ?¾K"ö>,®?¯eê#ø?{îE¿é?֜†QD?¾XjK£#?änúM}P'?'¶¨•'U?w.ÁecÒ¥?'—5'ÃF?ÖÅP_F•?š…"¥W¤?å6Ô8¸?ÎdÈXÁ.«?dŠ.Sç¿?i5"ïj/?Õ¦}úùþ+?Î^…ö"^†?èëâä]¯€?Ò'뽎ý?›yÌæT$?¤î¸$·(ý?Èá:ÑüÑ;?Ð0"@¶mT?êkýϤ¢?¯*3Ùlš?¡à±ë{ã?'ÀÃeV,C?ÂP"†Ï?­3Š8V?ë(¿x¼?°©‹ ¤Ô?sdøç­¯Ã?qRj¥?ÃL59êÿµ?°¢8kÚ®2MIXED3FGL J1408.0-2924@t%܇Tó@>'Z³R¨À9®`À48À;±£|qk?ó13ú-ƒ@pù½EÆ@|¾`xe¿äÂÛ­÷ZÑ¿ê(߀6NÏ¿ìû+–¿í»ÓáûvUNASNone?äX–`˜àÑ?ÆÝz©\?Îà:t½c›?ÄÕÛNŒ?¿zØ
r¯J?¶q‡¹î?ØI*¿" ?Ë€ÇnF¸?à^p79kö?Ë n¨‡Ò?»çԁÖÉ?¼[ܾ¹0?åC¤ú~i?²3ólɬÝ?Í׳¹3?¯,^ëŽR?»Ý{p¹¦?¢\ª³™áB?ËÄ0KŒ¾?´•úF»M?æ%,5'?»>œë*'h?¸vwOlx?ª2ޗ®¦?æ9|s¡•ð?ƛõè,­;?Î%1…ç"«?ÄÖ`¹'(?±é¹T"€®?«vjÈÿ@p?åÏϺN+B?Çl@ó¿¯?Ðø¬'2'?ÅQÙ[Ñb?±	Ÿ|aÄN?±`PÉW]›?镾œø°?©è5\Mö½?ÁÙ²EYrÚ?¤_֟÷f/?¯=MÍæ—?—ß;ª]?àõ¹|Û?N?°òފ~8?Û'yQá°E?°®M͵?§h¦®$ø?•]äßH9MIXED3FGL J1409.2-3743@sø!-w1@6¢DAxpTÀ9ÂÏL
ÑÀ;•e×y¿ïݦXނ@1›Â"¸Ú@—Iÿ¨lE¿ç<Õã™9o¿ä•ìÐj^¿èPâèÂø¿ïÿ‡{£©,UNASNone?îà¬yßÙ´? ßï|á8?•+(	ÏÛ¢?˜¬ThTU¬?~''(K¿?Ž(²‡Ä]|?îyˆl '1?­Aٕ`?—ûÄïÏ)u?˜ÔòyôQ?˜Ó-'ýÈY?¥ó¡f±S¹?ë{·4Eh%?¥-CY@ïý?´é¸MHd?>¦6"˜?®q!µv?–îLl‡k?숪«\1?®LÞRCÖ?£ì(›uSú?¤K@ê,¹Y?µå¦\{?¦c²[KD?ïSŸQí?Dnÿ±?"ÄíW¡E?…®QâuÖq?wR¦>»K?}ôŸãbu?ïŽíÛ)Î?']¸Úáê??zÄû~ÝFë?|iÞ¥â ?}Äíòª4?‰½¤ˆ,5?îý¥ü1?"rÂѨ¶?£¹=ª®µx?:º|mWÕ?—Íá[
xæ?¯z–"?ï-—ãzÓ?‰ïˆÓ<—O?qKyëd8?rªØڐ?–NˆrV"?‡dXóuÔAGN3FGL J1410.9+7406@\ﰉ 'R@DòF¿2/À9›ÖøjÀ;ûœGÉÃ-?ñ(ÆGÍt@.rÆÆù@Q_Vý"¿é÷£Öâ¿âEu³"ô¿Ô?Èå.þ¿àOœ&€ŒUNASNone?î"Rƒ–´?¤'*¿x$?—oH½RE?›_ÿB`?–fÔþÓ
?•ÙuÁgÜ?í;XêŽ?·KØÆî ?«nLO>®?±, <²ú? Ü%M:Ô?¥|éjÕEs?ëaÿMõΛ?ªvª,šÛ?²@^…Ø'Ê?ŸiÄI-Œ?²¯§	/-ß?¡žïÄ?ë"×üçØÓ?µ5AÚò¨Ÿ?µC:c|qÙ?²~pLð!?¬<mD?£.ÚSù?ïL]âÅn?ŸÈPºxN€?'a8à"?–Þ{ÐÛÐ?‰¶&a¬U?!QBð?ïCÀŽóE?šä:y9?Œ;㇮}?'[žIG?'ÿìS4¹P?ˆ_ìè }?íÙö8€úç?›Ì&'C—?£׌¹úG?'û ä€a~?ž¡‰Ïv•?+ؼhR?î>ãö½"©?KCá†a?§S[i)±¢?˜\âSþ¢
?'ù"°Ãƒ*?€ç£ûåċAGN3FGL J1411.1+3717@QFȟ@¢‡@Q—hƒöèÀ:nêžnëpÀ;ü jÓ?ÙÛ3tì!@
¾¤B¿î@ÒäŸý5ö¿évâ0Ðò¿è×Ýú#k¿åÈ-§iL0¿ÉÛ9B†UNASNone?ïß ¹›º?n›Îhˆs?ZOt€/8E?dßòÝ?c8'Òš)?cvÕñÿ°?ï¡Mjl‹?'½Þ=%?uä{{–?'¦l'?yu4"e7?€ô6ÔÈK?íîüÝFy?–ˆŸ­L,h?–ùÎ(:³e?"ÔBT;Ö?¥"KpÅ?'w—_Ya-?ïû2æ²&?–›_2
Åñ?'(Äë
ö?‹'dx£7?",7&ÃõI?;Zîñ?ïóêž))?WC><Rv?E%®Rwü?Qgk+—'i?K1ڋ={<?Joʃ<?ïßYÚðY¢?r\êP4õ?_	oi5
?e¿aƒw?a!myZRë?dK(s{>?ï³&Ԟ?ˆ¿žÇóøt?‡Í:ÕT`?~ììi2é?'#˜›Š
?'þ=[ÍՏ?ïÖJ/V¸Q?rY]ªJM?f"eÁ†Ž?f7™ÐpMI?c°=­0«?fÛëûcªAGN3FGL J1411.4-0724@tñ ä¶1@I3]9—À:†ÖHv'À;³c"GÁ¿æ¶twºæ_@ñGÊDj?þ]Û O@Z?¬U#I»?ᚌF'Š;¿â¢át';¿Ñ-•ÇIwUNASNone?ïçÞ-ÖÄ?c#(WnÈ&?@'7‹ÖÃ?<Ĉ>'À?dECcÔ|?bïÔÓ?I.êq?"½"h+£Í?w°l¸pºt?'¡îkœÊë?zƒn¸Y4?ƒ+Ãdݑù?îâj,æàA?‡ÿ¨9¢?µÇUG7Ö?~ˆÏN‰´?"×Ö¸€[ý?~yK4ú,?ï+¥º†›‡?'nÒ¥ö?}ÖG»þØ?€(PSÏ?"¶Ä¤i"?Ž¾Œåx?ï÷½Zi?O¤â/aؚ?.ªè"—?)Cv
pì?KÚPÚzë?N5¿Ð"ì?ïߧHêç?vï¯J²3?^«§ðhÃ?nÜ5ÒH,'?a›"øš'€?f{®óÛú?ïwË°x?tàIþ½	?6#u@@?o7'Vñáª?'ŸHØ¡â?e"l
‡¹†?ïØkå½oÉ?h	µ
ýê?KÝUm?A&UhÑaã?pNlƼ
\?f ÙP#–AGN3FGL J1417.5-4402@síÒܱF_@0&s>»ýrÀ9W€•ÓÀ;h"¡T¢?ؕ0›JÁ@&"~…@óQŸÚÑG¿ä'DˆÆ¿¿ãò[/Y=¿â{Ë¡dÐJ¿îØv°zJŽUNASNone?隑Ë2ݒ?ÀOÓOÑW)?ÇzZúwé?¿xsö9q?ÚîÉWê{?á3>%?çÇô5q{î?Äwx²nR?ÄTïêø˝?¹ÈŒœí_?¹~}¦¢U?¹"y‡¤{T?æþͳQ¦'?µ
˜6ýt?ÊUe­Xé%?²'h™Å¯?³^Ç	å0?›Ó½4¬Å?å»ÖŽ}Âà?³ZíÂÚi?ƨC^,9?±èvÆü?ĉý'ªÈI?¨¶Ü™?í³ë{Â!?®Àoç›*?°è8©ûͧ?­x펤£,?wíÿ'Å­J?v¡}íWc?쨸í2›?³DëÎÊI?°Tò3òGq?¦mˆ‡"t?¤ÊŒÉ°e?§•,°3ÐA?ëc
—;N?©lâ™w;Ê?»xûŒÂŠ?¥AËìñé?¢ßvzÐ?ÁŸwHÅ?ì`4ˆÈÓ?šñ|jÅ×Ì?®F‰(
?•»Îêâ¡?«¶.c‹WÇ?'$ë+c"TAGN3FGL J1417.7-5026@sËË)^ž@$9¹×ý'wÀ9u΁eÆÀ;7E¶Ãv¿í‡‰½AZ@
­^܄OÛ@âZߟO¿ë!ǕLÐ5¿áuV^¹ýE¿çMe—¿á÷¤DîGUNASNone?ì
Çö6?Ã òî
~?¢M@øp?£k¨[¤?¶'ùµÇ?Â~¼Å(ú±?íïv¡r"?¶Y±â"ºä?ŠJƒ±ÐÈ?—sK‰è·ê?ªuòét«×?³s:ÆΦ¯?êÚÝ/+ÍÊ?«:H8CŒs?«›?Ŕ~?—ÍlxÜÝ?»[v¢wç?¥rìw̐?뺢3­<Ë?«^åʑâ€?|ºö?³ß?yžö}Ý¿Ñ?À/ŸâŽU?ªÕç;ƒ¦Î?ëIfÊÔ?ÔܲY?H?~94¢É—?ƒÐt'˜ª?Áè›0-Öc?Ô6Ø©ÏÇ©?ïr†ñö†?—Tû‡X°?qd²pÐٔ?~™bò¨{w?Š«ÿKñÓ?'ûôÑ¥Xý?îb+yÞò?'¥õý°Šñ?•'lÐd'?'™£®´›?žžx%«‹4?ŠßïÂy0?îºûýÎÇ?‹™áÁe5p?W³ào${¹?M®6²j
?£'¡!¶#·?‹*w_ÎjÞAGN3FGL J1419.1-5534@s²³œ¾à@Ê'ÿÀ8Úoõ—ÇÀ;õ€J=;¿éݬý4Û@ÏJ€Æ@‡·ßªÊï¿ê˜úpQªJ¿ê~­øvHÝ¿ãèw¿êÛqÒò´UNASNone	?î›
þ×r(?¨~W~)H?†Úc)è?ƒ¯+/8fÌ? Ìéx
E?¦ÈEÊ&¹¯?ë1½Îhi‡?Åcí÷P?–ƒzðÍb?šé#»3+Ø?Àx˜W¥-w?Âò½Pœ¿X?çâußë?µË€éÁǃ?º4"þ-?£Š-'ÿ€'?ÆäÜ9á<?±<Zy@?êÉú4Žþ?¯åc¬‡9?é(µšC?z"ƒIVyI?įi"ÓäÄ?¯•.%l<?ï~x¿•"?•]ÖbaA?vë
 –©Ë?|mó8ŸkY?"æšø@"m?êšÄ¸?îÎÿ/Ü¢¿?¨®"£˜iü?}VD¹"5?"Æ­AúÈÊ?žÊˆÛÎuÙ?¤®E+»í?ìxÞG7eâ?¥cËG	Ö?©S	^ÅՄ?˜%À=y0Ž?¯-ÃÌb?œ'Æ8"™?î:çnÛø0?"ݶülQ×?cçHCÉ?\Ê®çjý	?«#Å«;?"‰wÎAiAGN3FGL J1420.9-4615@sê±[W>«@+¹ò™0À9'Ùe5À;i@։äñ?Ð'ÝßÄ¡/@
Á¬œU¶–@›¥^¿ÿ¿ë"¶å@a¿æñQïê¿ä3½6¬º^¿êÌádßR¶UNASNone?íÆגÍ?³¾ªƒÎ`‰?¦‡sQ[g?ª@3M"›I?›þ֏Š?¤	þñ ?ëÀ¬à?¾?ÀOÛ=x?¬©ðIŽ?©ÃÚ_yD?³§g"'	?·žµøŸäa?ëc˜öRúp?¦¤ðd!~?¯"=à"ÜŸ?˜9çÔÑXA?µR^Ö,?ŸÒ¿GV•^?æ {؊è?­c†ò~áR?ºÀ>­\<?¡d&l½?ÈöqG&@?¨ŠD;?îa=XêÁ™?¸I‰ÕL]?¡ þýFsI?²*r6¬¤?'–Vä«JM?¡ÆtZ+?î´ðúw…?¨´¡]¸`è?'~­X]ý?'ø
iE?—ã3_‹¨V?¡P8—?/?î9^GDH?—‰myS?šÃÈêª?‹§Ë˜?žŒ$-_H?ÅMÙP	?ìªôs7¾?"|ºÉf§.?¦ù(ñ÷å»?†Öʈ—F?®WÝ"óZ?ÍŠa 	AGN3FGL J1421.0-2431@tzzcslß@A¿"ÀiÀ:…îÁêÀ;²';ýP?ìPó/›@Mk›Y:@šÂ?U*?àZ¶_ևê¿áü»yµšù¿åÀ/@Æè¿ïÿ÷,OqáUNASNone?èÊX¹ÞJ?Î~ø·{?É®
Û·\‰?Ìù–âã˜?™D'íbJv?©qJ>>^r?چxú¦]?ÇÙ·â?ޚx
þŒ?ÇòÎqƐ?»}¦3…éd?¹E@ä½'•?ãOö@N?¶,]귆y?бáxoAE?³žw¿?Â>ý6!$=?¯$jG»c@?×Çä¨$'?·°hAr?àŸ´¯ZÝ,?ºÜ£Äë¬â?»æ
òˆ"Z?«ãÿ…)ø?êûҔ•e?ÎBí\ܜE?Á$"³rM?ËQIÒ9¦È?˜‰LÛ«?´VŸf¨¤¦?å…ôm˜}?ÂVûJŸÇ—?Нð^ð¯?Á³ãzkß?±X›ÑlÝ?¬_à$îKø?ç£9ÿ¼Iƒ?°Í'¦Ï<]?ÅÛYHà&?«r8^n´ä?·/}p¬?¥F¯ÎЍ@?æToüÅÁs?«Âkp¢Ÿ?ÐeýþъT?ªà§ÉRÜÖ?§‰=–'?š'fa¸öMIXED3FGL J1421.8-7920@s3.œË}AÀ1;'`4PÀ:0«ÆÂǐÀ;¨Ò3>î?ð™@Ù9Í@0Ç˱ç@&@tdV?î àç?¿äªÔÚ.×{¿å½'T«ÓÙ¿ê«';…UNASNone?êdÒ¿óÜ?Á<t|v?»ÝzøwS&?º€¨(u'?°ûïS}?­ïLFd?èQì""9?É1Ãb|I?¼Ð\Sé?ºDʽËJ?ÀPîîñÌ?ÁŠ!›J?å"l†ï{?¹Pbê—P?ÌZòt§ã?µìçÎ1±?º¦¶ß5ì1?¢w>ÍÔ?á*K#{†?¹Ü-Rs•N?ЙfSé?·",þnc?Ê$©oG?µwF3E[?ì•ÞV7G?º‰ðéH?³°¥'Ãó?¶Ñ˜7¸?ž –l¶?œŸÏ
617?ì'vçÏ?¾Z]ÒNÊ?©n;?©æŽpÄÙÑ?­QÚtG~?´`.·&ç?ë¤{2XöD?©cÆ_0£G?¸¦½Ö{&†?¥vÒ§ÿ¤@?¤jÑ*
²º?¶£±½ñ?èó¢)
:l?ª  óûÆÓ?éÃYØÆ?¥»ÃZË7?±h‡™? :÷ð‰AGN3FGL J1424.3-1753@tÁëíúCþ@CԍûÖ¥"À9äZ#bØÀ;¤Wë‰P¿Ún,£¢%@1s0Ï*Ë@c]a#Ü¿é\~éjl¿ß'"®iÏ¿ÞÆÁk«ÛÍ¿á§ù´"û-UNASNone?ïõw`=4?Lí̵?;'š³Ù–Q?2ÃCþ†Õ?La1öKß:?Gyþ_,Ï?YW<Û?Š
Œõ&¨?v‹Ÿ¤Ù:Z?{*~…hó?3§ù4?ƒR¨Û·9}?ï5lZ5?†$Uiæd?'zVb)AJ?qÆ4Yb¡?I×S-?€x~ Õ²(?ï ±«*²þ?†¤žk¡Ÿß?e®–H.×?^Ž€*™›ò?™3÷Ë tL?…¦UåpÏÏ?ïü¤¥U(j?3è@ôA?%"+
[Ó?s™2bŒƒ?0I¾›•?,\ËBOÁª?ïÛ·Ln(ä?jU¥Êº"?_ŽæÆö¯?UŽ¿"ÛÁì?d@:º\y?ePwèH-?輪¸\Â?pš3º›¥?rÖab{ä=?cÍՉhƒ?y]‡0VÑ?g:ª¿Š.?ïÏ0Í°Õÿ?c—œû8û?OÖï™qºl?:Í0Èw÷œ?tl»N§U?bƒo+"AGN3FGL J1427.2+1610@'.'O"}@PPe¾ ºÀ:¤.™À;ÅÏASCÀ•Öé±4@;cÃÉÃÙ@O?ƒM¨¿ê/¨+º÷¿èƒžNEn…¿æ‡iJ"Äe¿ïÿqñp+rUNASNone?ïø´2æËë?Dä­Ižy?;·OþÁÂ?6iÂ]7=?>§?-X?<ž÷9fÓ3?ï›óBGH?Ž‹ñt|?v—Þ%^7/?…ñÓ`Êy?{n€»Ðè?'OõϹ?î$˜Ö¸?˜°úÇ!‹B?Ÿ!
è¸?‰âBÙ-(8? M/ñzÐ-?ê'¦'"å?ïVܐí¬?'î?…ž\?i5Éc×Wû?t)³Ã"|h?'ý´·‡_=?cŽÂ;~z?ïúÖÕÂÈ?>'»P˜¼‰?9kó*pø)?4·¨kû?2VŠm…(?0׬ȩé?ïà…"¶…°?lú¶µIP"?\Äu<!K?]Û£ø•Äø?a¢iq¼?b¬Yãì¼?îØx
8ú.?‰¨-²Ëà?–smÜ>"?ƒ°rm¤‰?Œûڋº#v?zx£\Àe*?ïåÂ)·?fJP0ô?'UƒJ´¼?:0rvrš?hÈ¥Ü*0S?euný/RAGN3FGL J1430.8-4434@t'œàu÷@-•Ã½Y'CÀ9"Ü%/drÀ;nú|2€†ÀknY$	@ø¼—u}@Í?†'Í¿ß×ólàf¿çIš†\.¿ÝvÑӜʧ¿êYIä5Û?UNASNone?ïfEâ7m*?—OóJttD?…Gég{þî?‡¯º'…?&žqˆ³?ÈVª?ï2kx°&4?£Z"S?sŠ+\6!#?zO¶éi2?"Ð=Å2?¡ÿëè?ìú6'ì´Ò?£Ӊ+Aµ?¦b¸èÜ{U?–KÁWJU?©ùÝ죺?˜å€wߊ•?ïÜã<È*?—¦VˆI?4£¤kþé?DDˆ-~?œñÕ
'Æ?—ŽÑÆZ©?ïÙ«ú¼––?ŽƒÅɂ¨W?eP—J<ð?h>L\ÑE?aèšA5?œÊlƒº?ïÎ
꿦ô?|/ˆÕŽSÌ?[ÞÓjŒÅ?VûóŒ,v?rÕÑçìs?yP,‡*S?îû"±¼6c?Œ×ë±5äá?''É89?…A&Jsiû?ùAéB?¥³žt•?ïÉ.
è?u:é)|?"9¥»Í?rz¸&5?{EÛvɹ?tú1^B½¬AGN3FGL J1431.1-6425@s—¾ß¤@À؅Ó7ëÀ9K¼šO¡ÿÀ:þ¹™aÝ?æú¬ä•T@›5sñ@»Ÿú[Ñ¿æWþŽ]GÑ¿ê|˔WT?¿ãÀ+Ê^3¿ïÿÜ¡"œZUNASNone?ìTJq,+ò?¿ÿÏ-¥)Æ?pM¹›;‹?s¹&¸Š¥R?¼XÐÚ+7Å?¿¶šÜ9Ò4?Ö)Š¥,l<?ÑOKJðÙ?Ã=ãÕà?¸—×m¿À?à%ë4t"j?ÏÑ>‡¶Su?ç-_$0iˆ?¸.-²7A­?°ÆMÏé"H?œ|F'?Êç\‡·¼<?¶QöÔ['?ãÁ½nØGL?¶î'¾ÍÊh?¶8i2[i?¤àÁúû¿?ÒîjÖ&Ž?´¶0ã~"O?î>ø‡Kõ]?³þ™ÛÃ;¨?cSc@|À?dò©JO¦$?ªÛAUqå?³Ùv4÷¼?ãUÈÈAˆó?ÒQ.~§?º¢.NÙ<?²ÒP"Û‰?Ò«âÛÆ©Œ?Îa½¿é{?ëWþˑR<?­J˜	ä"Æ?¥tçGGH[?"ópÆ(Ó?º…–‰—ï?©ØÌÀ?鉐šõí¶?¥E¦úÁß?³ŒŸã,,%?–Ó·Bãu?Àm£¥Ô? »ËÀÚ¼MIXED3FGL J1438.6-4209@t5K}At?@0lˆçš®mÀ:
xë¤(iÀ;fûéðÊ?ä	©`¥Ì@+-Ïqï@'¸`.>¿ílŸæe¿ä½4ºƒ¿ÙSÞ%²
¦¿Ò¨"^F\[UNASNone?ïÂ7SJ?‡÷Y€^f?sßÈþ,?…± à$Œ_?f	k¡×0I?kõ푘5?ï$ú…Üg?¤¦§"
?"[€|
Á;?'o⬁)–?'N`hÔ‡?žâ\÷"Û÷?í‡A¥'Êm?š°=âôx?›ç´×#%?ŠµÑEè
?©˜:uæš?"œðe_)?ëKcj!uµ?°›bª¦a?•n¹Mv?Ÿ\ÑV
A¡?À1Ā<?­Â3­
/?ïìÏllîH?ˆ3Ðl2'?PYo´î?Y¾'ï¢|z?V·—L"?ˆD0Ìõ"J?ï¼î¥å'P?†€'õV'?i‡ã"'¯…?o‰Á×õ£œ?tÄ»,M¨5?€Ìw9ã˜?ï.ސ)ê?'…n^Ã\ô?…f9¦ry?u×ýÒÞµ?4¢þ?y6W+g?îqõ˜?sÖ?"¹ÀŸz«®?+÷f"L?‡‡ÐbfN)? Êªúé5{?Ž²ûüvnØAGN3FGL J1444.0-7033@s'ÂzcsÀ#r-"ÁÀ9æÆ:"‰À;™jZÀ†<¶¿š4@
u_þmY@–­ _¿æU¶ëè=¿éDT@(4¿Õ$8܌ֿê-h(»éƒUNASNone?î4ŽƑ?¨öÃužX?'ÙOنjz?†tkœ7,?¨Ê[QŒ?¦ñÕTaª?î©ì¦Ã	?©rLô¨É?tòøD?‰Í›oUÏö?¡r±¯WI}?¥§ÎÄ&i?ë¯+Zæo?§$ÌÓÉt?§ÉÿfGÊ©?'KÖa-ê?¶¢†ð»³?¡ÖñŠcŸ ?îñk(SA'?ˆí=ÊT¼?"²Lê+n¬?5´ÐtcD$? Ö›+	Ü?|ÕÌL_¯?ïTÒۍ7"?º8$ӁÄ?u–z¯Ž?vÚfü(þÿ?19 ?ŒU°ÂLk?<ç£#?˜¢–cgÁ?gæò7ÌgP?r¶¼ö,Ý?ˆ¥ô*e­z?"ä˜l*?î"ÝÂà²?Ž´¾ò?"Àpt¼}e?'tƙ—¹?˜ßsÖWQ?'±mʶœ?ïÀ7h!&–?yfNR²->ñuº¯ë»?ѬíÙº?Ó:šp²,?y`W€`íAGN3FGL J1445.7-5925@sÐKÛ ¥'?ÑèxD4b]À8¼~Ù$À: ^ØP?ґ£¥zè@
~p+—@»;\_¿ƒ‡éÕY€Õ¿è%D
y‰6¿éW"#žô*¿åc}äd÷"UNASNone?e¬:šì?i>…´Mç¢?§S-þ?°	AòeN?îyZ!3¬U?°]ŖÃ='?®ÕG''
†?´…T´ªo"?¹»ñµ.º?µÙHpD&D?êÛ-f{Æ0?Àñt›w.$?Å£ë­¾?©t"†=ðq?Å[FqBQM?°±Å+
O?åcÅhÄ(}?µN»¹yêÅ?Â)&:¸sá?ºß¥ÓŸàí?£BGÛÞN?™šÏϋ˜û?êA'óætÇ?½n"Åh?nvÙ|‰S?yc3}œ=,?§ÛNJ?·´<Ý%ìk?îo»r:Ê?·þÍeEv?ÃH¤O'Hù?Ȩ<{²Û?½¯à‡- ?²ü;5œUG?çwÚÛ5ùÀ?Ëh;û5?ͤ·"ç?®Èà{
ê?Ð8 ôº?ª0†ÀÚîQ?ã²Ä>?²ŒÂfYŠ½?ÈåV¢_L'?À Zí¦%?¡"ÓFg<?Œ›,˜n´.?è´}"óþs?À…ÿbî"OTHER3FGL J1457.6-6249@sÌn—OßÀ2ô™špYÀ9;ÛmiÀ:Ú
>¬ãù?ì^bq`@žžô@™G€r+A?ïË&´A2¿äI
¾À«½¿íñÛØŠõ¿àÆ\_SUNASNone?ÏEÕq{?ÈhFŒ;?×Yk-ܘ?Ëÿ»Eªè?ÙáÓçjª?Ï8|HOû?Ò'퀇µþ?Óa4Cc?ÈìñKmwä?ÄÛóÞV?à°ÌìàÇ?К+°O?àLÀ
˜?´†W/'GÅ?Æi'û‹jñ?«ÄXνÁ?Ô1êÈ$5X?³zRÉ©ìH?…ûhQß,?´ÒÀ6'a'?ÔÊr%Gž`?Ë™B0Ò?àùH¾H¦?ÈOº¹‹Ê?ÚJ&DI±?Ìä÷OR?Ȗ-ç¢n³?Ãz;J ¸?ÙjÂòê~ö?ÍPhHúÖÝ?à!ÜN¨0?ÖGµß~ö?Â8IÛÉÈi?ôOAJ'?Ö "tÊk?Ñ
?°*eë?èrQ('™›?¬&Añݕ?¸"ä›"? 0yAà?Â)©éë8?¦è¡ÍAR5?Õ*L:§W?·''Ñ_Ú?˾w…®¼R?¸Ç ²ÐgÛ?ÜöxJÔ?»¿³Öþ÷9MIXED3FGL J1457.6-5355@t÷zö@d@æK©K¾DÀ9™'W«¸€À;	……`ý?ÛIÝޘ¸@
1$¢e@Y^ðá)¿ç|m(CãQ¿ëݞc­Ï\¿Üb–#S¨Z¿á灇»0ÿUNASNone?èÓVØî‡÷?É͑mÑÙ?ˆÊ£Š…ÀÏ?Ž!?²öÌu?Ë%úcfŠV?É@÷"ÕR?䇧Uç4¤?ÓìSÙN™?¤ñímëÐ?¥–a$äå?ÔRs¤VOÝ?ѓMÙÁk´?èÝ
T['?²R¶'[Û
?­"Å£Ã?žÌ(߈–[?Å+šsÅZÏ?®T~fË+±?æË
mŸÉ<?¹#Ÿ\?ï?'û'ù.?'ójS,Ž?ÑJ9jëí`?¸•×Ô»ú/?îDZe¯ºÌ?³AËé'M?rSÛ°"?>î"1o?©oéÀ*Ã?²zxGûœ?ëÿ¥wH`í?ÆX¨˜e'?"a•çËe?š¼R¢x[?ºÿ;ßÕA?ÃÍê0WX#?í«'g†?œ²ËOäÒ?˜1`'Y7?‹ä9ޚ•ó?©.Z×?•ŠÎdLg?ì!H¿XèF?£q>"…û¤?•>3†.?ƒÚf»8aY?¹¯*v1pÍ?¢©ž®Þ#AGN3FGL J1458.7-2120@u)u\)@@JŸ±À9­—1àLÜÀ;•ÈFUNç?âƒJEžp@†úc
@»Å@;"e¿äËOT"š7¿à®îaᶿåí?}̒¿ïÿ°yÚâdUNASNone?è*›´üÌ?Ãf6o§ü?̜Þ<Ჸ?Âð"˜ÂjY?—óº©2©?"Ecì¡nô?Ñ'Üê§(?ȵȯçv?ãœòýÁ"é?ʍÀrvj?»ítžH¼?»/Wd"n?èB>5g7?®.L¸x(œ?ÄÓmŒÃu?©\§ú1?¶'÷%&Z?œnR8Ê?Õ'Jº?·ɎÔÅ?á_Pd
Zf?½³rŽ¼?À_ºeA"_?«ŽÊ¤!´?힘º ?µ5Ζn?´³;–A?³ûhÛ=?‰>}™GŸ?†ÖǬºN>?âb|ï¿Àö?Ç2Ga#Ã?Ö9ï¸Mþ?ů}¨ïšO?´ÁÖåÛ?°³ãc:' ?ìç~²k*?£røã÷¤?¶,ø‹¶dÓ? ¢Id¤¥?£w–þHj´?ŽR*ý×6?å}ìá%…‡?¯WP`{?ÐÝdU{BÓ?°`ãf­?°› æÈ?™3z^s†MIXED3FGL J1502.2+5553@W2>BZîc@Js,­'À9},²æqºÀ;îW"KS»À	úf9oã=@‡Þ@ª£ +²¿å9_¨Þí¿èëBó^uÆ¿áÎÒǞ̿ìOq4ÿUNASNone?ïûNÕٙ?CSúVƒ?,Å·»5¯?1—se6r+?9*®"Ù2R?;&©Z¢ž(?ïÂBÅøG?Ì#¥¹œ?kžáj³9?xd±'à?q0mÎ=#ó?tN~Ÿä}–?ïN‡Çêm?€úåæۋ?"¦dTԝÆ?wˏý
ò•?‡·Ô| b×?sï-Ë£®?ïð"èn'®?eÈüU
I?Ëv¨ä'? úÉË=¾?^7Pâ»2†?eŸ…G!â?ïüU2ƒØ4??ê8V[ß?1/ƒîeš?7S'=þ÷?(MÏû°,?+ÂÊ?ïé%!çJ?eãÎfš?T`òÖÆ#§?S=©e3?Y'Ã%÷—?_ÑȖӇÏ?ï'Ͻ¢I?Kt;žä?'«7tã;?{ǵŽÕ3æ?yBÒ5¹?eD86l?ïýá¿oŽ{?Ci»'q¶y>¸PB^íG">íb>½9»|?0Ù´ž˜1?CheAGN3FGL J1506.4-0340@v,ï~=Á@F•´¢3œÀ:$³ÑSDKÀ;}fÿéYË¿Ùœx,r¶@
²…-Hc@ªyßêᶿà¥ÿEÅÜï¿ê^k¶Œ·¿àÑ@ÃzÏ»¿âaZÿUNASNone?ïÅ];^>¾?}V"¤ŒK?O(ù(J??P»Q\–D?ylC‰•,?{_	QE??hº?•æG@]¤?{¶'Þ;'?'ÕÕ§"û?É	 ?…SA	yj?í°2fž^i?™dç
ÕP‹?˜5 {Ôr?†¿óãvŽP?¨âIYçÝ1?"ô懹e?í£×B»Î?šâñMöÞ?sÿÒèk»?oaQÖð½Ç?±¡JÃÄ?™ø_|Ü,c?ïóó°øl?[ºiÚ<?0³ü?­?4Ž®ìc×?Së݇KÊ?Yv§Ž'?ïۊ7Pú?p<nÓ—Ì ?`ªbf<úü?^u˜xQ^c?cËfî´À?g1·ÈWÁä?ï@èrš?~¢¹OÚÅF?'¦,>h™?rh ´Û0i?YuÀ‹Ý?tÕяˆ€?ïn•¥KÝ?vލ=ˆl?ah$æ™—?Oˆ.H­Ã?F½LÓÎ?uƒšyGzwAGN3FGL J1506.6-6219@sÞò<ÈÞ+À¹§Áz‰3À9g´ör2À;¼(ßó¿ÔZë´æÉ@>—Îé2?ýµ¿©M¿ï»;µÀó?á<¶(Æs¿Ýª6˜K‹¿ÐQ¯ÝJ?âUNASNone?½à»?¨ÖŽóq}ü?Wä†;?y%H]t?«e1šH?§†ÖWèC?ê"7›ˆî7?ÊÇG
ùM?—>g7ÕUô? {ԙ—7·?ÃTªs¨ç?ÈI…ÍK€?ì}¬¦Ö]?£ç§ûy`ÿ?¢;ýÕTñú?"2Nã'*!?²ùÛ®Ôùž?ž ²I‹0Ã?íd?Ï<­t?ªŽ­šfúß?zNQv‡G?xÀُ)?³9mR?ªG'K']b?ïn2õÝ4?Œç(P}²8?kú4n±‹k?q݃xïZ?tí-c'+?ˆv%
e=?î¾[ߓ"?¼œ(ë?ƒŠ¸fð™?e ¥±¾?©vÖ(É«?¸§'Vü|m?î±fÝã(7?'ó!s'?®knÖ$ú?"«¿uœp?™$¸Ì-ÎA?ˆø˜çôÄ®?ïD¥÷Jû?‹
©GÛ>?a(‡"€o1?RLk-Q?›rZPވÅ?ŠpÎã'AGN3FGL J1510.2-5754@t›'·þ?À›ý6¡ý–À7Ûx\2/þÀ9öð{þ~ ?âÍ'æxð@™3& !@'qàBŠ¿Îh›!%‹ø¿èˆÀa•­b¿é8©F຿è"x±OÚUNASNone? §lŠÕ¢?Ÿh…‰	?ÃÞOv_Ø®?Ä&²!áãF?éýõZäÄ?Äû'¬(?ªAo'MB?³ÿ=	F¤?¹ðR[@?²òåóáÏî?ë8*ü'òä?À"pšiDµ?»´ªÊ¢Ò?¦=Ç'D³%?άÕd塟?´odÁ—a?äÞ5MrW>?¶Ö¸š!?ÅÔchžé©?·'}3q/?§ÚõG~êx?™ôfì3Ÿ‰?é
7ÑR˜~?¹|±…¸U
?¨"à¯ô?¨³ö°(¯Õ?Ê@@¨ÍÐ>?ȯÕ/ÇÃÎ?çæ±Ê_VŸ?ɽÝP}›â?¾@dß}©y?Æ(ΪÙC?¿‡_
	[|?²5‡Ö‹'ú?èG'oa?ÊÛàùï?ÃäªÂ"m?ªê"&ï×?Ïk¯Œ]¾?²Lޒuw¡?ã]›lCu?³áÝ,ÐÊ\?Σú2XV?»¥G¼pøÕ?§Wì?'ù¹Æ³ú?æáL؏'?»çÓ}.îšOTHER3FGL J1512.3+6622@Yò¬![š[@F•ÿŽÀùÀ:ÏDÁ~À<,)d}XÀx½VQ@Œ©-oz@Ô UŠ÷¿ëÀK÷œ¦Œ¿ÔÖr@Aí¿æ»™i{¢@¿ÙL…Ç2UNASNone?ï¬)"'RV?"Šx!Kk?"+-²ÃÆ?"_øì˜ø"?9N%èrö½?:Ýà×M&ð?ï·'ch§?"æ•dšx?q3m-;Š¸?'Ðl!bç†?s8á)otá?v•0,ÞOj?í¡¯!±?£~k\BÁ´?ªPöo`õ‰?¢QíÈã.?—(1=ôö?‰ë,C¯÷?ïíet+©…?a[9?ôX?7è p]?‰(w…¹?b̵)\æ?a%o'o2Ÿ?ïÕåÓaš?‰y'£iï?tbñC?s?‰f?¯U^$?%D©æNߖ?%…ÃírsÉ?ïçú;<c?g­_-¾Ó[?VÀ³A"üª?\†ù€jt?[!X)¶¬€?]û¯øyx?îÔDžÑ£?—¢Â'U:l?œž¾+%F?—Hèjü¼î?±[ë­Êh?vKDÏûCð?ïý"ó¬#y?3)]¬Ã>ÔÖ ãQ',>Ùmä½ör?3
|ì	o?3=É¼³AGN3FGL J1512.8-5639@t‰ÞÒ?ðxÆj²üAÀ8«l)ôÆÀ:y*GÒ&©?q»I*ß@X"©Èeà@³J'Á¿ä7hˆ:ݳ¿èc#ÿõªM¿ç®Â¾+g¿âb¨ÄYážUNASNone?êmD4ž~l?À'¨µE?5gå?"ç6Ž*s?Å8þJ•r?À.63æÞ?Æ;²¯PvK?Î4À"'?¨Ñ'×ÈD?¡µûû¾›¿?èä1…*™?͸¼tôÕ?à—@ð¤Ý?¹\˜¦¥QÑ?¼$Fõ÷'G?¦Â"X 
?×Èla8e]?¸Ç"¶Ï´?æ'(:K?¸9Rs·ª?v5@‰Ÿó?q""qFw´?҄ډ'ª+?¸r¼FS?aÐÍ?ª>ìJ§ª:?uûËH®f¦?ö%1B>?£^0‹-Þ?§ó"ZPh?Ó­åcûÌ?Ô·^ìI"É?¯`Dþ֗ù?£ÏHñ0½?ä3þ"Ҋ?Ó_‹Î!X?è{kÜ ?´ÈÆ­`çE?°T!ZÇÜ? ·}OÛ?Åè?â÷!?±/¼Þ§œ?ë[ÄR{x?¥@ï¤â#Ö?p#¶E¾§?])À^M"é?ÂÓóf?¤ûÀ€8IžMIXED3FGL J1513.3-3719@t½Ï€Ü3r@1u)wȎzÀ:Ž»üÊÀ;¯=×Ñã?'{,¤ë@¨>?úõ¡à:õ¿ï£ŸB"¿?Ə`"¯ì?Ô?~~¶¿àMÔ)–UNASNone?ïùNFEDê?D£W¹‡?,_—â'?%…›Ð+y?C¯o".Š?B¸ÙÞJ÷?ï>:Y(v}?™ñWT`?›þõGi?Ñ!½Ò?ŽÕk›žEj?•)¢—˜X>?ï
'F|!u?'¹ÍVš?…n¬óšj?t¦Å1'?"¤XJ63?{/Ð!ÊæÓ?îÔ˕®í-? õ+Eìø?s
.Ô	E9?€,%Ìe`? Q Êz? WlI!?ïûȁþ6@?6$'ÙpX? ♚ž?´'ÕØze?9J¤±'ÍÏ?3Îß=M´?ïÂiz©$¸?{AÍú"15?h"¼0H?aK5Æô?r¹ä«y_¤?vHj€¾?ï~nI×?s	גI(s?z¤­úô°?h<˜5c2®?ƒY›8ÀdÙ?hÛùQ™\~?ï ¬'vߨ?FL­Œ?qJäCM¿÷?m{ù£U?~^ڜ¿L?vGÖ.ӃœAGN3FGL J1513.8-6250c@sædobÀMݤõîÀ8SŠÁ'À:Ü»ÛãÁ?ÜA¿¼Ý°9@?' *læ@¨V¿ªOt¿Ôîà·ª¿é"K"W¼¿êª{GZBÓ¿ãìÕò]UNASNone%?ì—JÄ1Ú?²''?¤™(f˜¾½?¤Ïó6²³`?°ùÞ$T?«fXé?
?áü¦à4Q?Ò0dvÍê?µ°0Z¡óA?³*àP
¥?֚¦(7?Ïï/o¦£?æ¤ë¿n?³ÍÿÏŽ?¶lJle?¡Ì×èb?Ê/YŸX U?°®¿\iù?àšåeN…?´9JXљ?±‹Ìø!×o?¦Cš+°u?ÚgAøÈÔ?´e&Iíi?ïÝ#ËÐè?›…ÕsbÃÝ?€ÙA'ßÌa?€c¬e®?—Wº½ZÝÕ?˜=Yâ%x?餅!HÚ?ȉ?—£'ë?§ý"€¦Û+?«Õb–¤Ñï?ÃnŠY,8?ÃYìtKÆ?ìmÕj:?£Y
&WT;?¦gÝÈìš?"Óþ·'Þ?±]ÊÀR÷ç?ìk"¥š?è³ìµº%o?¤XEèÑ¥? äf45"?ˆlžÌ¤×è?È÷GÎåo ?£¦ygO8…AGN3FGL J1517.0+2637@DD¾´ .@LÓ!ž¶9À:֖»˜ÇãÀ<®U¿ôŒ•YîÞÅ@
Åë Ík@ÄÕ"?ïÿ‡à'/ ¿ëÿe8Çz[?Éc G†¿äO€ڋkUNASNone?ï×ìÆÅÕ??…Í·Z))5?8X­	õ·|?Ic•¸Šnj?r"å‹*°?…qG'µ?刺)K'ò?†¨VÛ4í¾?tiÎÀ4ë?{üÇBG˜Þ?xŒ[¾N?|ä‡!œ³?î1¤Ïúöù?–ª¬,ƒ?•$œb8é²?Ž†°iÜëè?¢SdÊ蘜?³Ç×ÀQÜ?ï¸nW1Ñ?™ÕƒòÁ½ ?J)I?~?]{z'c?›¸˜ôiZ?™+Ò4Îe?ïóàbMJ?j6žyª0?,öÓ¬˜?:Q`ŸàC‡?V#m¢
É?iÛ7`ÎÓ¶?ïáâ׌Tž?k‰y0Xw?[r&¤ó(?ZšÝzÁ&?`d'BXÉ?bw°Ocv?î½'Wª-]?•6ÛA+YÐ?Œû\4çÆ×?‰˜Å3Pdq?™Ýfó¶ð?äÍÈÀæŸ?ïܜ*Ãx?kÒj&TŸŠ?1r!zàx?0(Vjä&?pšÈ‹ÿ?k‹*'ZAGN3FGL J1517.6-4442@t‡JB®Ñ9@%›î=_ÜßÀ9^dµ—&À;=_0Ϭ?ßÓ-‡ç@C÷¾½ë^@²m¹¿éBÚx1¿ä[/Õ@õпèhÁú®(ê¿íÿ:Ó*UNASNone?ꐧëÊq†?¾Ðù0œÄ¶?ÃñÁÊvl?½ò°AÝ#?Œ¹èpKªi?‹"ÇOŠW?éõsV†A?ÆÊa\*<-?·Ú±¼?´ ydáO=?ÀžÅcÞ?ÀÅ£Z/è?蜬ëÓ?²¿W£'Ý6?ÆHUë?¯v—6‡?³·Pßå…
?›ìc_Ág?âdऴÅ?¬£…LLã?Ȏ
E(p?ª#ç§ڔ?Íßó8O~?¨c9H;§"?í©ÁMm?°c*÷ÄU?±2eWó†ö?¯Žðª>ÛÈ?wùåÒR)?yÊE-aD?í\>Îá"È?¹yXÃ?¢°"­Zë?«@\ûÿKl?§Œó"ëŽ?¯KÞ'wš?ì]lÓ­?¥?&9-PÏ?¶ukëJ6;?¡{¯›0?¢W
ôº?Žû€º0°%?ê:¿¢Jv?™î^&²?µÕ'>|JP?"÷IŸœ˜?¸Z
Ã'‡ƒ?"Kå9]ÍCAGN3FGL J1518.2-5232@tEš¿4@‡;…èíÀ8ÔÜޒÇîÀ;ëÚ¯
Ÿ?ôèøo"@ŠìËÅ»¶@îÿ´€¦¿Ý;|Râ¿áhʧ·?¿âōñÎB¿îìӍ†:íUNASNone?ƕš"XÈL?ÀS9m´äN?è*N]01Ì?ÄdŸuëXm?±'X	^?²ï"`6|?ǎOü%T?Ã9f~MÌ?Úb¤	µ
Ž?ŕâªÚ‰¤?ÙÖ3øCâÈ?É¢»RM|?ÚÒ1Q ?·îpùâI?ÛóyU<®˜?¸Âƒ|.¡??ÃïiO#ÿ?ªÎ¯ÖëáD?ÔgAÇdr?°GX'ä?ÚA¥šú±?·† B=,Õ?ѹ󣝠Ý?¯Ð<^y4?Ù0HsóS?É:ÑÚu#?â¥Q³§?ɃàeÂæ?¥·£fiCû?¦I!u^À?Õ¸{7"ýå?ÄýS)•)?ׯõ½3_?¿™v¾Û?җSν?Ä/»É3)?åÂÝhâ}Ê?²&Çjc?Î
EJ¯H$?®ªî¬u³C?µÔŠ#f? ;'h§þ?ßk'Fl~Œ?©\‡íÚ‡?×#UńY?¬2K  ¨?Ã"–Ç›ú6?šTHbMIXED3FGL J1525.8-0834@v,)³ún@C%žYò»À:©Yš¦	À;²X'hLð?ªf€‰@À—µ=å?úM]ÞØh¿ïÿܬhÔ*?ïه2X&?ßÔUq{¿Û†fÍz­×UNASNone?ïõÀð[ÙV?Q¡ê'®Z?0wpïF?(‹"Èõ¢?P|AUFÇ?PÅIWə?×A'>?ŽõIµÒ?|T(|Èô?ƒ$§Æ­Iâ?€45ÿý¹ò?"O'SWs?ïÏ2'´%?…"ó`Œ.?†Î×ÎdzÊ?x¾…œlžÃ?'>­ÃOÔ?"°Þ? ?ï™úMʟ\?ìÁšûª—?df"%?äI?tÂBœ«$?"gÇÁøkã?ŽåŲ R{?ïú´W¾ý??<\8'?#8(‹;?l~‹Œ	?@`£·
U?;²æÓ¦^8?ïØ-/°i6?nN‰'ø?b[Ûº"À'?[Î2ŽVÊ.?evô‹Õ!4?eæý~´#¨?Q'‡P?wøý˜ù¶è?ylíXþ\Þ?jNE™ |¿?'Ü5?sÖÉ	ÊP?ïâ$Ո™?j"¿ðç?[¥¬Yà?ZaÛN]K?`VÒ®eé÷?aвñ••9AGN3FGL J1526.3-4505@t˜Éšé$ò@#Bö@c^À9•xgðª"À;FKMÜ?Ú…`I
]@¥Vôƒu@#—Á¼M¿é—Gý¿í[ÌçFB&¿ÐG#H•¬¿Çh(ˆ¤UNASNone?ᅩ0êƒ?¡þ´Ã?Màß6sØL?M².ÃdQº?|}˗¡||?¡ø£@ȃ?îÏ~³œ?¬a'ÕÒà?yf`JHâ?‡—[«ì:M?Ÿ¶¥š¹J?ª:CmŸ?ìû›^b-i?¡Éxœƒ_Å?–ëœÜõ,ö?‡yEÕ7°?²h=ÕCUû?žô¿Hïvà?íK§¨ì?©{U…w?[hwE+b??lf5a‰N?µ5%š9×?©d6ö·+ü?﹕ÛIl?²Ø[\ƒIÝ?<5oՃ
?=ý0Æ?€ºO'ù•??²ÚƤŸ?ï©Ãã¨f?‹,þ¤`?b¿-›"i?aŽ"=É>?€ß;Êf'?ˆ>‹zݞ?îôÍ&¹Ó ?àè?'6׶jt»?t'~Xz´_?˜JïQ+øŸ?Œ$Ôb¼W?ïJŽó3¥?ˆ;cHfÜ?[{KLÿP?XÄM™PP?"öl瞀?‡ÄgÕOåAGN3FGL J1527.0-3804@t܃ä%¯@.¤ÎóÀ:š'Í¥:À;€¦'F•ç?¦oÑòlÎ@6žK…@¡í`@1ž¿ä†¢Æê¿ì'Vv{ª¿É€@›ëGP¿Þ°4|UNASNone?ïÔxk‡ÉŸ?}µå=¨ ?6!|¾™ë?5SSb^Æ?ta²vܦ?}	R´äÀã?ïU­l<ò­?˜ƒ7ÌWÙq?vaÌñ®?{áBè—_?c¾Õä½?•"T¡iˆ	?îµw»£?•›h<.£?k?ÂwY4?zwõ¡›?¦ùÞ¤vӂ?'Ê÷L·›?îM%3…v?›ø.ï9…É?`tG–Î	?g(KKI~Ë?ª&hPt­>?›dñ3‡¸?ïï¤PŠd¦?vF~'ìš?&b3>Àô{?&ýWÕbî?]ëR·Pò?v!`Ù!Úq?ïÍS¡Mÿ#?yfUØ Sb?`Œ²â]0F?ZÓD3NÚ?qÕíQ6‡?uNšIÇ9/?ïM¹Ã
d?€ ùfµ?|q!¢€Ò?i§O¼¸ þ?ŽÁR–?|&Kaß?ïš/³»ž?vÍQ41E?]_֗``;?Q´'j¢=1?…ÒyELvŒ?u*êî*ªuAGN3FGL J1528.1-2904@u9ßý`é@6m
$F0fÀ:ˆäö=öÀ;¡míCdÚ¿ë;
ª‡½@
–cî<D?û%÷@=ݱ¿ëΜ¡n¿ÝÑäy;Ö¿¬¬àÐ
?¿èº³Î,UNASNone?ï놏q,?bPŠ¿¾û?M:–SƲÓ?Párµû'?ZU—
™ô?[TÁž&Žc?ï–ä^"J?Œ´c³ÿW?tçÌãÄ?yÂìÜÄÿ?¦!|ñP?‡7¦ÔMq8?îÅ)»÷M»?QI×aÁ?ŽŠ H†!?"VRàu?˜¸9r?†Ðç¯>V?ï10×Öv?'²cöç«à?I'*H?Rˆ˜ÿŽ•­?™
SÇõ™í?'wR<w?ï÷i»Qòˆ?J«iÐÌT†?6ýˆîHZ?3;³ÊfÐ?GWŽÆ²ë?FYçÖv?ïۍÚ@L?lSD;ìYÎ?^·{ïÄ?VÀlí>K?eg»õì?ftä5Иž?ïayùÚæ°?ƒ'
YkEd?'(oäØý?}mɳÕ?…y—_¶'?vÞÜü=¹?ïÍ¢íw´?k›Aì?@BýyÑ+?8«ŸCBî?w&)–¤R?iùy6KcOAGN3FGL J1528.7-2247@u€Jßø"¼@;Evš'^À:™ï)îçÀ;šXKñp?èÁǒ-ù@
ێ	Ãx:@ðßëb¿Ùz£QJ¾¿â-J¹6Âà¿â™3ÅÕ6Ô¿ïÿÆ×âYUNASNone?&äà?Ÿc ¼¸'…?œ®Qè[ó?™·ãÎÊg"?‹g¦fãb?Œ{òôç?ã'ÄZ–<?ÃÒ([Ç?ÓÕPÿÌÔZ?Á׬öSêõ?·l™)öã;?µÑC'm?褺¤•?­Å"ž
xœ?Â՗ŽHúè?¦ï7ŠÁ%?µ/)¸¹"?¢Æ?iZF?á&¢¨>×?µkî¶Ð×?Ôè¼aŗÏ?·\©®|º?Á"ý5ÓÕ?¤Š§Ï—vb?ïhµ+V¬?õ™/ø|d?†1ƒwò"'?‡0g\ø¬ä?–žnÀÔþ?€ãŠÜ˜îã?êËg6ð×ï?²½ì}·ÓÑ?¾ŽŽ»]þ?¯$ÓE£'?¦-Wmxt?¤PŒûʓ?ì*"?@m?£À.84•W?µϳúy?ŸW´ûß	?£I,§zn5?'¡âW<k°?茧:Î]?¢E±­:?ǎÑtQ`›?¢N?ï}R›?¨úHUæ-Ê?vh'iAGN3FGL J1529.5+6733@Yß1)Ë«@EŽ'_ét£À:ÄŵV­À<3r"XÀ¿ëg¿p³@;P'¾N@å
ŸÁ%û¿ÔÌ!nî'ï¿çnéÍíî¿ây|ˆD¿àÕõÀêtUNASNone?ïͧ[à6È?"$«|QB?vŒÛ9†èG?ƒ¿@!Íj?Dû¶6®ñ?D´—<Ã7÷?ï¦fT%yÀ?ˆI Ch?sP,Øñ_?€=D&F ?y|©PÙ³?}Ë&×¸í?î
'6>š?y©Cá?¦_¼&'ð?œÕûß.Û?'bÈÄvß?ߐ#Ç+?ï¸×'2tÇ?yF$?cû?F¤žù1‡?D\Õ^;?€_Տ&kª?xnöã¾å?ïê'ËÒ¯m?y´tº¾?cçãqÞxt?y¢RgæJ ?(Uj´ÙN?"ìÙÍ[?ïâ>ªØ?hòVb¥?Zm^4b\?U컸H?`µJ¡ý&ð?aJEd<°?îãâWùf3?—gÐÙ'ÍD?œX¯&pB?—Pú콑?|¬T>Hv?g
…'¼0Î?ïöJ˜Á??Og|ªéf?"ë™8RH?ž`Ÿàèå?Q
nx¼á?N«Ã¡ì:AGN3FGL J1532.0-2618@ucblvK@8ºˆ&«À:#Š·~‡À;†@Ú»¢Ù¿Øp™Ã@ú¯Åüe@uí οௐæº9¿â(GŽMÏÛ¿àç¡Ú…È¿ã¥1 Ö²UNASNone?ï÷½ÏŒxQ?Jݗ†£L¶?9H¾X+ݼ?6­Ãâœï(?Ddb·yŽ??D‹Ì
£??ï†Dâ!­?'Âë×¼Ûa?wÐ¥BóÜ7?zæQ8׸?'†tâIȋ?:›–к¹?îù"¢J(~?Š¼µÇZn¢?ŠÙÏù»?€CP
;ÙF?"`ä¤ãW[?€ë,ñp?îGö_ Ø?'›E½º»F?pDh¤¬	Å?eΨgRv?©†3'°ÁK?'ÊPGurc?ïýtÞÊ?2Û¸ð›aÜ?"!Ã4\_'?Å8'cœŸ?,fëì´eÙ?+ÃåËÏLÎ?ïÖÒV›åq?rÉӟ*!o?`ؘM5]E?VÈàôÁòJ?hUÙ:g?ojáá4†?ï'Ú'–[?uLZÈÌ?yOvˆ8?pÎ)½?pk?}C@_Ê?e×و®x?ï'kãd$?pd.åóS?Z °CÑ?E)꽈öä?ˆ6O­À~?n°ñ¨ºûêAGN3FGL J1533.8-5231@td <K	ê@"]¶ŠÀ9m'Y4À;
Vìu߀?âÎApQ…@KšÌ>‡?ÿrû?{ëß?í•ï{«ûz¿Ù˜Ù]Ý^¿×(>;é©ì¿åŒ2 2²UNASNone?ïy\"?HI3¿cò?rót	qز?p7Gg?ˆDnҘ)1?Œ˜QKöCV?Ýz«mú?ÖÇjÃÿYù?²dm߶ÇB?±3cìø?ÝìdÜgcU?ÔÑ2#àý(?ìS'ãÚt?§Zm<wQ?Ÿ<¤Å‹>?ïð~²×f?µ"MÞ½â?¤,ëhÀÊ?æ*a6Â?µå??¦"k;柭?™ÛÔùá?ÐÚ°,O‹¦?´òYè€fÖ?ïÑGуsp?tÍV"sÞ?[:ØÕÙå´?X³üE7?pa	º†?q!¸è6†4?å®;È`´ÿ?Õ»ö6ŽÃŽ?«ªÂ÷?­ìê]-7?Ñ.F–ߢ_?ÒýõZäÄ?îŸýT6U?"ÇdœÑvD?èJÕÜØî?€‹¦ÛWDW?/ýã^ù?Uúb¦ 7?ë_T­üŸ?¢3<ÀÁð?£ðqL?ˆöúµÍ³¦?»}gä¹ã?¡وÇå1MIXED3FGL J1538.4-4656@t¢þÅm\û@¢—žÖÜÀ8•;!>>)À;còPë?ìºO¡þÂé@Ë­MÖw›@˘¿Ô쬿èo‡]"V¿êúÌ5¼ê¿ê"Îà¿ïÿ¹€Œ#ÝUNASNone?î…jç:Èd?¬ýx…/¦Í?'=O/úÔ?"ú2œÆ…ò?žSûßòµ?©—`6$?Ü1 Œ›?ËL'ÊóXÓ?ÑMJFÜD?ÁiõîG?Ò·'(6ë?È{÷›
:Ÿ?é°÷AF?±½å"žý?·¨Þ¦¬=?£pM'Û5G?ºÏgN÷<–?§‰Qۑw?Ô}—ÿÕQš?³€Qgœ^?Ù8
O@Qv?ºy4±bŽ?ÒJZ°ê\ï?µSûfÔzŠ?ïiwŒmOþ?—tÈ~ßY?~LeØýª·?€àۛž`ç?†{éî6M?"ÖÝê"ë_?å³k›j»F?È# EQ»+?ÄHï½½D?·‰NE»Ô‹?Äéaԗ'¤?À‹¸\ŸµŠ?ít–Þ²?¢ák^U?¦Õ¢^>n?"j#IJm?§Óšõ£Öj?™N"_8ŒÉ?ãߌ†Fç¬?¬µ™Þƛò?˔ÈP³™?ª8!ûðC?Äí"¼?¥ýd‡M˜MIXED3FGL J1541.6+1414@7­ ÝD@H2`=WyÀ:eøg…JWÀ;¯ëí#"j¿ß±‰ñ—Å@
#Ïj¶Ø?ÿš¿5Š{¿ï §IŸ?íx‹dw£Ð¿ãW}vö¿ÞÈfžùœUNASNone?ïôÖm×Á??JÝñ^ř˜?509¦tñó?-¬€ÏÅ?Q^¹`?Fì°U€Ò÷?ïmÇ"‹<¬?"·ÀÍÅX*?H‡÷¹?†1ižCe?ƒF.ǘw\?ŒÈ}žœÿ?ï¥ë¯L?ƒ'E¡Å™?†t
ü£Î(?sJ"‰û?"±VßÅk?|îB¶ùô?îEö¥¢ç?¤fE}dd?¡nž
šø9?¡Â°¿%j?"d|ôê›?'‡EYF/?ïû
Bf_Ž?5ß®½†'?#ÿ<í©þ?ƒ$}34S?=–LNq™?2'À0¨t?ïÕ
µ9!#?uCÞpŸ?de³ý_Ê?gz] 
î?fŒ–ß|")?l-[nïَ?˜ÃRG?r­Öû?z6^Õ±‡?hÁª6Ï9Ù?'»êTÜ¡?e%EG|}>?ï»2;øÚ?svçr?mÐèS­Ó?dŠ›ÓôG?s~Öt\
?m㯠ÃAGN3FGL J1542.4-5911@t4ÿ'+¾ËÀ
-\Äüô³À94If{_À:蟔…]¢¿ë—7'js@2·7dE@Ðà©-`¿æq-ãÀã¿å¹û6(¿êdV#Ö§u¿è¶u>_PUNASNone?ë"Þñ‰çí?º\n¼‡k€?¦¥ŸÝ¦€?§`<iˆqã?¸8…˜àÖ?µŒ%çÀúú?繘¼ò0¬?Љu£ßÝ?£ÇDõ‰?©ö"þF›?ÌSëD\%p?Ìñïׇ2?æ—%s ?µ¥×ñÕ+&?¸u<h_;¯?¤é$õ—l?ÉhÍÉÌè&?±rŠùþ?è´/Ì:DŽ?¶þïr‰ÍX?'ªi²¸"Ú?€šÍe
Í?Ìš2_'|?¶½«`ó34?îo21¢Ü±?¥YŒ­/Ë
?†xxÍ÷8>?"µíi"Ï?£n¾µÄà?£úÝ5
?ìØÃöøŠ?"Tî™Ñ"?è8Å
º?™×%Ð¥ó?´ÿÒ×g¯?À
ÔÏû€i?쩆¯=\?£hßÃmª2?¢¬ËV~\"?'šPñX?±]dÞ´¨T?ž®MÝÈ)?íg¥*ÇT? –€œˆçd?a ¦–Í?XxŠ³&M?¶ AÐ<ä? mKóHŒŒAGN3FGL J1544.1-2555@u‹ÁÝ!ê@6œŽ:!dÀ9/Ô!Tä^À;Y 8ð?õ'ÏÐã1é@qɎ~ÞW@Þ]@L÷*¿×Û«Ë(œ¿çêeÜJ:®¿å¸y™§¿ïÿ§¿!>UNASNone?ã—ŠCT,?Æãh*òÙ?Õº`Ø¡±?ÆØ8èÌ)0?¨» ›äŸ?¤ÏÔò"¹?Æ
Å&¡e§?¾fB‡ÂŠ?æÓ¯1'â•?Äcüÿš?½Lü)~ ?½ó7sùeÌ?à–¼çÉʱ?µ¶†Z굫?։À½?³›-°äÐ)?À"߸·Â?¤ìAÔ÷?Í-Kä@B!?ªõGþçê?ã€I=$'u?µ	©«mS+?Äя)S5‡?«¡
Íʉã?èÐ\66È¿?Ö©ÚÚV£?ÊÖ ;°k~?Ãd"¦Ã¤?Ž~îÁ•ìN?‰× rB?Óäµ Þ?Ã3™a²ÄÛ?ã.$Œëúÿ?ÅuPÍU'`?º[HÄ­"?¶™Gå‰ì"?æŒH5$á?±PÍøÇ?Ìú[€YW?­­÷…Ä5á?±©‡02
I?™b‰WÅ]?ÛVÈ%j•?¨—¿Hz?ߋÃäWH?¬_)žC~X?´uÏ؋k?š|™MòMIXED3FGL J1544.6-1125@vC`¿]x@@~Àð¸À9iW²n}À;Jǘ°eŽ?õºçG!}@á—YÎR‰@M`@1ž^¿Ájàܷ"¿çà–>¿æ	`m?¿ïÿá&Ž4UNASNone?ß	œ*Œñ?Ëq–ZÊÑË?Ü|¯+Ǧ?Ë·͋õ¨?±æє^{ž?´Þ¯Æ‹þ?¶§II^?¹Ê˜â[÷š?꽆v?Ɛèð¼?¹Vp\mðó?½kf*^?ÝKè]™Z§?´yâÛÖ?Ø£M£ˆ ?³txLÝj?Ä!"ÿâßð?§×%åC›s?¿+³âðû€?¢çA¤,s?çªY|Àg[?²gå­ÉpZ?ÁÀÀ…äÓ?©ÃÉ9Œ—?䬉˜<×?ÉqyG+?Ó»'pc?È¢]竏)?§ZÒôÚ?«¹às:€?ÇEºbG?Â!gÈ°f?çu¼€à?ÆÇ8Œ+ï?¹<oTÉm?¶¹Ö™ñã?ãÒéN¬¦?±âÖ²®Ý?Ò/Œ
Ëò?°,t?Q€z?¸ª…]a)ó? âèOÝ?ÓKZؓª?¦Õu3{?ãV¬Zw¬?­ùhƽ?¸#)1Éó÷?ždõ'ÖÆeMIXED3FGL J1545.0-6641@sîἩiÀ"Á'Ýãu†À:'Ns*šÀ;r3#Bû?Ñ…cñZå@ûÉTrH?ú¿æŸÜ©º¿ëÖ€BÓ¿å"x†/Ú¿ª5.é€k¿µ\]è­AÜUNASNone?ïïOá?œ?d÷"ù$÷¸?"A<ו^?&ãdé«1?_[ŸEÓ?d0psx"G?î|s;ã?®Î‹.jù(?Bh K9?†–0(ŽU?¤PM¬Êé?«ƒÊS#R?îüœšø5Ô?‰{'àyV?ƒQS®E?qÚfóÇ;?–Ãá{6€e?"ìÈ Ô]?ŒD¶,?†¡DÏ6
]?-±*–?Aþoá0?Ža"'t;?†}²ž¨k&?ï ¼k*ÆR?µÜÓãC?`ÕÏå6ú3?'þˆ"`5$?ƒ›qB‡îÝ?±èTŜZ?ïzmú¦Ç?—ì¿M¶«É?h֐ËÞm?o&I5î?‹HÀS»À•?"ØÎd†Ð/?ïÝWs§?u¼¢‡"Ï[?tz#:J\M?dð³ê£+?‹«QÍ\%?qŠQ¯J‡ð?ïè‹DʽÜ?[©C4üï§?.\ãš4½y?1"ï>ãi?eŽìÕöS?ZZFDsÀAGN3FGL J1548.4+1455@9¡ë¦¬§"@G–a©É"À8õªõâoÌÀ;g8¿E%?Ü26Âù~ @Ø"´Šá›@å­_Ÿ!ï¿Î¾¬ÒË-T¿á™n·©á¿ãJŸfy¿ÝT{eY©UNASNone?ï÷•(×ËÀ?D>R3Ú®º?=ml¸ï`Ú?4îZ/–p?Bô¥žR˜?=4'kM?ïzuò pù?"/q¦™-ú?}ØKŠ‡ÍÓ?"åüQÿ?'v]‡I$×?ŽGü*?ï&œøÚØå?‹æ:ú*h?†KcÏ´èè?~‰Ä–½Í?®÷£ê?ƒ´"±MK€?í'çZ0'Ý?¡
¹?õáÝÄہ?‡×,±•¸?®V™q"k? n
•G?ïûJ_Zê˜?4W.C?2Ìd¶Ò©I?)	êü› ?2àžÿOÖ?)GÛm¬kî?ïÒ'sG±?v¦—|–Ã?ei'ó9¬u?hNވ¬¤?hnùä±:¸?pIÖ(¼Dé?ï›ÑV<?w;yMªË?x39¡`?qS¸˜ÉF?y‡C3d%?kiò£?ïežÝÑ,?Ù<(›œ?xН¿Öˆ¥?cg}?ÙM?Š/ù¶È{?Nzuµ¹^AGN3FGL J1549.4-4832@tªó¡LìB@ìúi¾
À8²³8§{À:ÑuúÔG¿é1©´€@~A…†g8@ïš@]".¿çòŒEYa¬¿íc\‰ÿÙÑ¿Ó«›q,Šo¿èp³hÅUNASNone?âCAú‡O?Ð&:¹e?…z•iÖË?'ÐLƒó1i?Úͧ_¢Ic?Ð@‡"´W‹?ç‹c¿_b?Ð8|ݐ[?¨à4­• ?®¢é$vuá?˚ffD
O?Ì3éü!h?ã
Ÿ¿'?¶µ-
Ìû?´¸R¡ i¼?Ÿµ^;⓺?Ô»á;³y.?µ)¯9(?à69ùÝq?ÄÔ@݄š?Š¯Æ<öç?ŠNR ó»Z?Þ¾
ÙÔ¿'?Å	šúRþ?æƒ1¯"F?Íð¿	.–°?®šЖ=?ŠzY'Å?Òzâ82»-?Íæ_´µB±?íphló?Ë?¾
68:?"¡3.8Ö?¡%x¥ý,?¯(ߞéæ?·æÐ%&=?éא,)öì?«âYdÀáì?©-x…¹,?–ŇqŒ¦?ÂVa/3¹?¨z#{WŠ?çÃ%aÁð?»>;¶ÈY?€œ""¡ày?sfh!L
?ÑE•ԙl?ºÿ
Â*)AGN3FGL J1549.9-3044@ueâ'@·€@2$<µ¬À:f6ýÃÞÀ;"¹
Ó'Z?éÞ~š²Ý@€n1áÏh?÷¦¿òÉ·¿îm~ÂÂ?ï÷TYb`·?»áéû—÷"¿¡Å«%.ÏUNASNone?ï®Òê@?'•ï³/+?H·Äø(ã.?L*‡‡F"Ø?'íÎåTÒÆ?'\ìŸb÷À?ï|ÊåÂ?"Y_I$o?wè¼L‡"?}þÈJA¤³?…
¸ªP×ü?ÉÑÔ	?î5ccŸ2?™
°Ji?'u"?:À€?‡Æ)8–F?£ï8¢&é ?•ü@ߗuj?îˁ0Ÿ¸ ?¡ÍgVšNG?" eiPýz?fqzËá?œ§7ä^>?Ÿ!'ÆW7«??	3õ?–ã›-^=?=ÔcæØ®?N€HyÏáþ?Ó5:­!¢?–Ëbµq?ïÓvù9?xvb¸î´?`Œãf¸äí?]M€R'™?lc`&Ùx?t*<›er?ïKSºà?')Erˆ?ˆ'ñ@m°?"Ëm™Ò?"•–ž ;5?Š+ÑÒá‡ò?+ƒ2ò?"u—"H>?€èˆvzëb?|¢;·bß?|UÙPØ ?x°•"Ð…AGN3FGL J1550.4+6027@W^qŸŒ¨@F‹ÙÂ~•1À:TcûRÀ;ïèwM>w?¬cª²h@jùÀöªÂ?ýƒ˜ Õú?'Wÿɸëû¿¼!`DZÅ@¿Éb>ÛÕJ¿çW
×ÈÃUNASNone?ïôt=‹ô?aE´€××?JUÛòh÷?`fC±¨ª"?C'³¨_¡*?=À7Þàr¾?ï
ªb"Ÿµ?™±ÍÁ4*?¶ïÀ¨\?Œ¼ë`ê.?ŒÞw"62?':Œ‹³œ?ï.)…×½8?†'«}lžV?ˆ •Ç‰U?~`Ýl'ä?ŒU´É9´?zK‹¥­Qœ?î¸^$gWA?–æ¡¿%ü?¬¥Œ'_	?‰*]3¨G3?˜G•äÚêÛ?›jäG´?ïù¦$Ü?eO‡6°¸?AÆØ®© é?e,r^ø?3ýBÿ€N?+Ë[ƒ¿L?ﶬ˜i?x]ϏÜî¹?sB*=‰"?i¨ `pͯ?q¯ÈMÚ²?q'_ewU?àk)?u3"CyÀv?{Q4Ä6Š?pžÇÍ$Þ¡?{¢>šv¹?cŽç}ò?﨓|@µ?tÇç¹|?x":ÀRc?eùçfCêZ?ró®²WE?kÙ÷	ÄfAGN3FGL J1553.1+5437@Ue3]$žE@G•¶Ü gÀ:&¤¯wÀ<y_gn¤¿åZ¢ÕF\Ê@˜•¸Ž|@
eÿ¹3=¿Þêø˝¿á÷d¾¤µ¿ä]ql¡5¿é©Ïzã1NUNASNone?ï•CVŸ|?³ÕÍHÔ?ˆ©øºÐñ¬?³Ù 9®½ç?P)Œ8´?Kv2Z?ïj"¬<*ö?•Âïíýãµ?ßrHÌ<y?¦AN¨$d?ƒ{¢£œ?Š2H]¯0?îw§Òþ{W?")¾ÈÛ¯?œW³Fô1?…Î5­‹ê?"³RZôJô?=–š%ý‹?ï3±-	""?ß,ïÎä½?͒Á?yûH™ú?'ô{»­Ù?‰öª@Û½V?ïµo»¤±P?µ¼$gv-o?Ø\l¤Xc?µ¼ã—0â
?9v•;â{?N1¿?ïÖNðî?o¨Ä»8?c¦­¯uUò?]ÀôZeM?fAlÒTa?h ¡‹V9?ïbºé[´î?'½pãY?‡—òòȬN?€ÕGei¯?r¥sshx?f}7ïÿÜ?ïáw½‰«?f´G?P"ÿ"!?Gvc¡Â?f>·²F¬<?d¶°%V6¨AGN3FGL J1553.3-0322c@vñýÞ½@BJ^Ý)5À9mlÓgñÀ;Q'TPº-ÀYsä©7@Zž¥òîJ@€p]¶¿é2ŒÚø¾¿ãå×;K줿ì2©J€q¿Ä?"úÐÐUNASNone!?ï°+îè¢ä?ƒp)yeî?u5‹µÒÌ?{tc3?rYÓ‡ßa?rl(@¿¤w?ï³Îü§ÛÒ?ûÄҚ{ž?n{ƒÍø?yYñ‰'Û?vÚöü	G?ˆxŐLÑ°?í›å¶uö?›m+åQ¢? ´_y}¾?;¿#	þ?¥†:)æ?ýhpãµ?ï£yAèá3?‰?òÝxX¼?-!Îæ<?ð¸r†à?‡'ZùûÎ?‰;#7Tºs?ïۇWD+ö?'VKÚ?bÊ`Pj®!?ƒP³ú?a®H"¤«[?'¡Zvz??ïåM¦ôB?h3yc?Vð53Ä?US$Ú?^t±TÏ?am™ãÝ\?ï'.Þ\9?…¬Umv¤B?l2zøE?}Ѫš,mp?Ž/Ã|%œ?y*aHámˆ?ïïSï㟚?]xàÌ<
â>­-S©ú>ÁÙÓë?w?`ª8;Èe"?]wÇC?T³AGN3FGL J1554.4-5315c@t"Ùè>B[?Ö-íCdٞÀ7Üݸ­[À9Øró<£?òí±ÔxèŸ@76³t @
 8ð?ÜÖF±rÜÊ¿ÞGh¤¯!k¿åZeCё¿è°Œ'ãRUNASNone0?UÒ›ð1?yì]3&eø?¹ý	§.é´?¹¹M'Ù}y?ì{'Ö3©?ºH(ka«t?"W¸¿ã?	YQ¸¬?È8ˆÊ5æ
?¿†æ¹‡÷?題nQ±?ÀšO÷äþr?°q
åóo?@Õ*s?È'ª?²gãgc©'?çð–=n r?³½È'U‡¯?©UÇg"+?¢ ^ò¹!s?Ã4¦kË;c?¬ÒUŽ,?靄øDAE?´ÖE»XÙ?ƒUWÌ¢áé?"–$ŒTÌ0?À{6l£—I?ÀµU•fa¼?ë"ÝeUÖ?Á‹0S?˜þ¬8¿1?¥t"©²J?Ð/ðU	" ?Àà0Ï"3ÿ?ç q>(&?Ãl(Ìk¶?¸¦‡¼íõ?¤a&3æúZ?Ë«.óę‰?±R²ü©û?æqàB ?³e¿ËÄ?¯X6-%·|?ªkßÜzèõ?Ã|EÃ%%¡?¤ŒZeØö?é+k,&?³""ùþTOTHER3FGL J1602.8-1924@vç#$È6@8Oh7÷¾À9Þ_>Sø¦À;eéÁЈ¿æcÊ«Æ~@l˜Œ´Y@€õs}¦¿ãþö,RÕ¿çIQÈt£k¿â6©µF¿äžÙ—UNASNone?ï ¡dr?…q¡ÀËø?XsY"ÕÉ?XWMG	?"ÉK*NFÛ?"+çm³õ?9ïv+?'#_´#;L?wpöð‡F?{ͱ˜ Å3?'bv^-?µö"çö@?îTèõ¢Y?•!+Ø«)?'\¬/G?GI0ó­?¡£!ôð£?,Ç}:dì?íÝ.Ìǃ?•øUéJï®?hÒÜÌa?`P6ý˜?°Vƒ	–I?•wI˜ƒÝ?ïð•F£¨?[«t;
?:6sxû'?5Jé]ï"G?Y38fK×û?Xl¼0§?ïÖDX'<
?sä¤øLù?a»]B?X؀%ÔvÌ?h¢¥/D©7?pM>Ã{?ïra܆9?w¯žaT?|^¿Þ9Í$?hß>»?…8Y"š!?qZªà†n?ïtÎEóª1?tQL1Ôú?R/Âݸj?@HØH½"‡?C;°[?sÃ{¼ÆAGN3FGL J1603.7-6011@tLƒùdÀùà`þG™À9è¹/a›À;k½"J¥@?ôèâ'Äb@hScTc/?ÿeþ>´Æœ¿äتÐgzÒ?äÖ©G¿Ø&ã&³ü¿ëMãÃçÔnUNASNone?ÔÓìÎlV?Èkäˆ2òy?âäÔcw§4?ʽ¯ðÀi_?µ‰©¬I:*?³6	)
u?¾ÝOò_%?­Ó7uG?ß$øLØJÚ?Èüˆhçœ?Ù#³ò=þ?Æz¸,?ÜÎÃl¦ÇU?»€£¢Ûô?Ú/딗?»&\Ô0?ÂiÛH)?©|R¥®¾?Ûp
IZ?Á¦=´ôòc?ߙzv$Ó?·­?³Ùí™´Ò?«Ú&Œè£p?ÞïèÈMX›?Í81Rfù?Þ#'/Þë?ÍJ¿â¾÷?§d)c:\Ô?¥Kz=8
Æ?Ò7ó	˜õ?ÌÿÅ)•?Úð§ru=o?ƊH=<:?Ò×eˆ)œ?ÁÝŘ{?çâ‡@÷?²ÓÝþœ\?ˌ]l¨Ûè?°ÌÄMf)?°00駯ú?šÌÑúQ?ä ëÁ F?´ ã˜áÐÏ?ÕMþu¼D¿?´aa AÄ?£\6Õ¡?"û`|û$åMIXED3FGL J1611.9+1404@;ÈnÁ~ºñ@DфV!uÀ9ÞÊ#¥ ¶À;¨÷ÇLZL?â~M±A^£@5»Gdâ@­_á'¿ßTû‹bZy¿á˜'xñ‹ý¿æÐB=šÈÌ¿àÇB+@UNASNone?ïÔæÇIÖ
?vRkux4?g¥˜æL?l?›ÃÛ¥?cs ÙýS}?k@¿Á]S?ïH¦Ú'‡?™\~BM?…OXŸ?‰ŠY¦2°â?ˆÓÆÁ8ýŸ?'ÊÒúøÔõ?/–Ï?•²°N8‰?"²'¼Úo?‡%ŠRU˜?š÷·t/ƒ¥?m Ÿû¼?íOŠqªà? XÒc–{£?ŸÞ
3uþS?•µ£'œX?«2CuÕØ?™Ý®Oçâ?ïô6gèi?Z^Ê¿?IKG¨VØd?Pû†6Â?EÛÚªÝß?M¿7š?ïǝ#"-?zq½Õ
?j[C=YŒ??k»´ˆ?n™‰vßL?sGgC&5?ïgêgð?ƒ‰!–œ?uŽf¦x]?u!Ã#¼?"×ÚåÚ?~6™p‡--?ïP`³%?#…†^I?†*®
‡?r_ìMÀX?…ʨ'KoÕ?ws}i¤ì®AGN3FGL J1613.4-4222@uû_ïJ@t‹e#pHÀ9p¦]¨À:óˆBY@ä¿ûÚOÊB®Ñ@cƒ•vI]@zs 
Ìã¿â,3_%ª¿í— m‰¿Ûš+ošl¨¿åÁü¸‰1UNASNone?ç粨x?Ë<!÷Õ?_1wàûò™?_É﬜~?Ði7.Èô?Ë6¤	'®?íÖÎ-þs—?¹¾Ú=E'?~6pk:?"9Ø!jb?®ÌOá
Y?·ÌV4öôí?çí8ӎ»x?µÆæ)rò?¥y<l>?"Šó«·=?ÊìͱËO?´zýûÖÁ?ìv•e­Xé?®½ œ©?6cž²¹èÀ?8§®\2†?¼4ñ4œP?®µƒ'cÝz?é€àšßê·?ÑÃá	y?SHØh6Í?ií¥Ü‡M¼?ÉÖQڃw?ÑÀ|·¶?ï.ât1‰?šþ#J̜?eÊӁ'K?uxT	*?ŠÁÆé›Ö?•ØM÷¼?íú]Ãnn?£ek·Ûb?'»Aƒ†?ƒb0óÒ?²a\λy
?¡­DÈ?îÏ[œLÁ?'pòLjˆ?"ON쎦	?ùý|µÂ~?¢÷öèœd?'hO£DAGN3FGL J1615.6-4450@u*™0¾@?û¹IbÀ8Ó%žõùíÀ:³ËE
PK¿ì@†÷ð*å@Æ4/²u3@~ó€jÉx¿ë`ûZ©Äµ¿çÒí!mc¿ã"T
"¿äÝ
ë-¿UNASNone?îͽlÔáç?¤±Ò ?uqqb;?z;²®™M? r;¾<?¢·ß|h5'?í²·3ÂU?¹úæ%8sº?/&tæ\?Šý¤cr?°Da—'W?¸2´Ö]…œ?çÇ7ì¢Íl?µ@›;Iƒ?´wÿ/¿n?£Øj¶hmŽ?Ƨ ¶Æ?±ɃִŽ?ê˜3sÜ?²=°ÔÐz¢?Ye4 'ÅŽ?Tdøb´Î|?ÅlgÉà*Å?²*Ѩ¾JŠ?ïš@H£˜?'Ÿ,â~hO?n?8Ž2
?"é+ém
}?àßG9'?‡Ñïzf?ï`53_ö?¡€Ö+z•?i½È‡Î?y®V{Ÿü?ÅàW?Ã??žAe™ð~?í&
ô¸?¤j%¶
'»?¢¼Ì-"tŠ?™¨.t`?ªâb]Ûô?› í³¾?íк	ѐ?™wÙ¿½ë?Fâzz«b™?;ԙÀÿÆ?±Lj¼·Uí?™TtmÝu‰AGN3FGL J1616.8-5343@t§—¢H"ÄÀ½Õü woÀ8ZÉX¤À:ªí"Ãq?äèKË@]ÄKžäÝ@=Žà-&Õ¿æÔ¾+Qðì¿ãy9Ó>­¿æI"܍¿ïÿÍݐ`ØUNASNone?ØyH?o?ÉXՕY3?Öÿj§òè?Éñøm
(?Ðëª@ìë?È@áÔhD?¤'Ó¿"²?° É#±?Û²¹¯æ?Ä®ÆdB?àݚP–Ï?Åj!¯°ºÑ?Õ=e}Ր7?¶—¿pë?ÒÝÙjü‹?²Þ§²wf2?×äÁ.g>?µàR_76è?Ç_T'ïù?°Üo"$?ԅˆSSÃ?¼æ^¯§è?ßËRsë4A?½M±#N
Õ?æ$çqyü?È;î8y'?ÇæÞµœH?ÂdӔ<7"?Ài{[bsµ?À‰Ï4Ž°?¼¢¥	Y?À¦Ñ'¦­¡?څh¶€c?¿gÛFSË?ÞVÆïÞ?ÐYÿ¡?âŠÂ«*Þ?³áÇ+ch?ÉVU§§N?«íGÉEÃT?Ì~àiÑn·?¯ûûhµƒ×?ÖNœ³K?´fˆê¸}?ˍÄó©IT?°>t¡| ?Ûꁄ‹%Ê?µ5P²´˜…MIXED3FGL J1616.8+5846@Va
xÀ@EX¤Ò²ÀÀ:1ùˆºWÀ;ÿ1æ,?Ï¥#\óÃS@ǐ:`˜@ʅ˿î'ßÞCå¿âÆm1ܛø¿ïü"±Òæ?ïژߛSUNASNone?ï퐷ÑE¶?jf·ªˆÍ—?K°ô1Bf?Rtb—í¤‹?W«ü:S?f¢RônO]?ï¥ùrXsE?Û'4?uð [?"¿‹Ÿ±
?wrV4Æ*y?‡€.þ4Ä?î9Ã맮Z?–@L™Â§?—†k`îy½?Š#6k?  ‹–Å«{?Döaî?ïÈ&'Ô8Ú?†.uÚ݃?Uù¢·³1²?w8YD3E†?vnUËÉúƒ?'vÏ Òt?ïøJ÷Êý??U&È¿íƒ`?1.µ<eˇ?8½qL·ÖS?F<Åꇢ?RV'î'·Ù?ïݪL' s?€•/ºk?aÏÀdº
?u4ªË%ô?aMãyÀÂõ?lpwça0n?ï#,fªã?ˆ ¦èñø?‰F6Òf3?€¿…Òjƒ?î¯±4ê?T¬®`s?ïûÂ[ã3I?Xwç¶È?+ZnÙbõ?AÖcø/

?;âH²üq³?TÄ/مAœAGN3FGL J1618.8+5520@U:rŸYÌû@E¹¿ðEwÙÀ:·!†b…0À<(‰hÉíõ?Ûrv¥"ä±@n@'â@œ?ÿIw¿áðÁ?·¿ãô™'ì3ù¿ãQ厾I¿ïÿo•þÉ8UNASNone?íÐZÞEÆ?¿ÉsžT¶³?®ô¦š-õ#?¿'K­¹V?€ã"`?ƒ|­$»Ì?äŠñ,Ÿé?ËDX×Tµ?ÒÇÇ=°~?ȯü<Q?´¿…Zî@?±êòM_»?èë;#†[¾?³ÀÖ?ÂU×ÃúÇ?±ãwH¶Ó?³úw_Dú? 4|‹ÉÃ?å*$VK'#?»ìã‡h-€?Ñß·ßïƒ?»bÚ«1Çx?®_û˜[8Ý?Ÿ5/RL)Ú?ï+.a½4S?³Tm˜ôS?—Uƒ33…ª?³ø·N­?j%"Ĭ_?n6úh‹?ìé>Ö/]?´z5ŸJèÄ?²Kœ•àB?±?ôÝÜt?šg;y™B?˜\ÐHSí?ì8†6îÝ!?¦Ã
,-úG?µyHÃͦ?¤Î»¥¸)à?¡…æ|Ó?¨18ð3?ìҁžv?žÒ²K•d?µÙjA•?›¤:²X'M?Œ"GêAÔ?'x˜M*^…AGN3FGL J1619.0-5014c@tÒy»­À˜?Ÿ¶a-ºÀ7á€hp+âÀ9©{rg%©?ñÂC@–ÕU‡pø@s|‹5©¿à2׶=r¿é'¡˜Êr¿èíçؘ¿å²8]$ÚUNASNone9?{²GWXà?{n$®‡©?«¶³6?´zZ'•zŽ?îZ˃?µ3͘~Û`?²¯'Ù̀?»âûQ3h?¸ ÷*}ß?±¸‰Þ`?ê–Ŝh?Áÿýρ»Š?º²‹Éªâ?¤p2T&x?ͺëC/Ÿ?³¤!å†kº?å;ºê¼?µSSR!/Ý?¾àâóª¶?¹'íØg? ¤öíy—?šÃÅè0­?ë"9?»ø€|3¤•?wèÜë°j$?¡¾ÈO?­Ù1šbßw?¸jLô{?íò›,Z•½?¹Qf‰Íl?Áö
2Þτ?ÈdôÇùº}?¾$•{@­?±ÀW›Ýä?ç½í€˜ä	?ËÛ`ZÖ?ÁáÁ.;°8?¨‰bœ…ÆÏ?Îl
SixX?²ΪÈk?ãìŒ_–µÜ?³ÚGÑÔ2B?Á·;¶9j?½Fb_G'?¬†üœ¾Õ"?šC"¬yh?éÉÁHÎê£?¿ƒA[",OTHER3FGL J1619.1+7538@[EÐ|"µÝ@A¥ïÝëÙÀ:ԛÀ»F"À<%ZÞrç~?âÀùɞÞÂ@~¨Q˜?ûg€)†¿ïõÜíù›?îã†tù§ ¿à"m¾‰-?Âs¿Æ»!UNASNone?ïö2¨/Ú?vÂÐ)b¡Î?MD\W?v»Á¦lՅ?4^­ä?,%‡g¢Ò§?ï¥ÏHÚ
?‰'óºÍEî?s»ÒNÏðe?PUùËÏG?y\‰Åptù?€\蝫Q?¢8
?ŽãÙpٍÏ?'{$TYh?ŒÀ×{E?‡%×2´æ°?tÑhs—¸?ï¹øæŸöo?'Ï=e÷5Ã?sÝ»š½án?ÌxQ¿ø?nK¢1¶‰?r¬'‹–=ó?ïäØÊåt—?«ýæ‰Ý?iòŠØêÊ?«þðKÝ+?#R7^åj?•yò¯RI?ïá:š'*‰?igQø5%e?Zœçõ¤´¹?V‡8g.ž?avò![t?c"¢BØë?E•'Ö?¯}wÍ0"?'Cx³l"Ù?€õô",Cˆ?w²ëÃf«]?a­€íØ`?ïóJ5B
?Z{­ñU?PÑr(/Ê?S
f_œ?A5Øòžú?Iáò	ºI2AGN3FGL J1620.0-5101@tËa\¦Ê¿ä?ØÝý ÓÀ7çÇj<"À9Éb¯ø€°?ñÖþí|l@_†`ÔV@[€YV³¿Ôꔉöt¢¿Ü{õv[žY¿çÎ3¹¸?n¿ãf1R2|ÕUNASNone?ƒþûëÉ	?~,U_Œ9U?ՎYduJ…?ΎЮ¿×­?äè×^:Ù?Θ#Ô+Ìô?§nNèöm?±º".?¯NC§A?»U	Ԍ%?éÝG€ù?Á3¤Pèâ?µU@Igo?¡8m¶$?̊WÐTn?³ÞWBd²?æ2ÂËÆ?µ°FœV[?¸eÝÙõ?²Í;€‡?¶_ó²I%Ô?«
7Ã].Ò?ê']Î"žw?¹˜…ê©	?z-{TßQF?wêpr>ü?ÖK"!þ‹?Ðw}rúüé?ä¥ÛJÁx?Ðy';|,÷?¶N1±oÏ?¾'˜q+?ŞQ>ÌÄ?»•›®Ø×-?çÎ¥{¾×?Æ9Çq³?¿\ô0)¾?¦_î×R{'?ÏfuïrG?±²XÕµl?ä:ÄT­×?³a á!ó?¼¢•ß®Yx?¶U…aŒ£?ºéçxŽv?£×"u	?é{‡¤"b?ºþóTdÊõOTHER3FGL J1620.8-5149@tø}¿H¿ô™@
6IhÀ9
Ñ­ÝÀ:oê3åàš?à¹+¤bd=@™Ä6%@»Õ@Ž»o¿ÞmW°¯Ï€¿í!]'澿CD?S)üT¿åµµAüàÍUNASNone?Øc¤›'|¦?Ë$FŽã;?wDü .ï?wAac»ñ?㟣º7|w?Ë:¸Ý'–?ÎK ðeƒ?Ò©	?±ïDB""ý?¯;n,bÇf?æ/T¯To?Ñx™˜±«ù?ÙÈFÊX˜?»‰@°
=?±ðyéê¯?œvçd"w?àû¾‹Q¾u?»¯"è\ ??âb´Ít	?ÉÕôð³G?u{~õؘ?€Ä£­4þ?Û{Lš•ö€?ÉÔg"ë`?áÐ.]$b$?η¤``Ø?r¢Ì
Ù3B?qˆ…'¬
¥?Ü2'š?ÎÁ:a>£?ݙµÖ«g?Ö™ảí?±®"[?Xë?©ï®þîy?ÝúÁ"Cû>?Óö"J¿Ò?åpkˆVÛ?¸°¢òú,-?©F*Ï¿ùÞ?—óèWˆK??Ñöc–tÃn?·#x'd?æčϝí?¿¿3ñ-?l€à#çr?"n'¾3Ûè?ÑpRq?¿(
B¤MIXED3FGL J1624.2-3957@uQ¢3œ¿@–ž^$x…À9 €©ÌÀ:³À~à°¯¿ª´‹P‰@×´>ág9@(‰ðü¿ç"[À×1f¿äEmG¿æ?d€¿ïÿá{ýɼUNASNone?Î`öÖdzš?Ç/36Á'?ËʨÎH€€?ÆíÍ«øty?áu»òú?Ïë j-Æ7?Þæ\%êã?ÏYÿóI?ˬN¹1ː?ÁЁõý·?ÓC|~M/U?É0_ÒRj?×ÝCÂÍoŠ?´SÅ1\uJ?Ð9ãý|(V?±*PaŠ€?×èØ?¶h ?´§¾Áäiá?Ì3Ȟ-ÁÉ?¸¯|E`?Èmt­j?¸¡f!"?â×Ê;od3?Áª,1ó?Ò¦£Ý@?ËÖæ]wT?Æîÿ Jçõ?ÆsûŽ2Í?á7læˆ4Â?ÐҎÄ9¼u?è¿¡:ͱN?ː@
˜F?¹s6ñÑ?»Çž9¼d?ÀGóùPRB?À4O¢ã?áɱt²?´'VéP#?É"ðð÷?«›P PmÜ?ÏÇ¥=@Ž?±/"´…á´?؎[$O&?¼	ïò/¡?»M·GCOO?¦3uxR!5?àOEi…nƒ?¼Œº<k/MIXED3FGL J1624.8-4233@u4®}Vlô@…`&±EÀ8ËAøÈÔÀ:¥Zs¿èʔŒ6@2ˆ9tëº@:×@H÷¿çD"8­¿èCÂöÆV¢¿æxþH𴳿楿l¼íUNASNone	?ì}=âÄc?¹	¹+ú¦?"V"Ùß~?•·T|%?·@rBßðã?·¥:Àì[?ꯖ!®À6?LJ²Ü‹±¤?•¯‡VEèà?›ÍS&åêM?‹¶Žê5‹?ÅTèøÚûA?ãZÍ
ïP?¸Á[l§2?¾«û¤"6ä?§ìaɐۚ?џfüÓ¨?´Ñÿ.ÒY?åñH=öš?»Åm\ú¬Ú?z&",´'?sÚd ¤,ö?Ó´Õr–S?»°âBw@K?ï/߃U+ù?¢¥¨"Y?{n`•GùŠ?€è8ì?"(wpäiƒ?¡)²Çh	?Ÿ"óV?­eâjÀT?~DÒ<ÚC0?"ÙðØ·êý?¡NK¿%'6?¨ùèÂAq?êVèú!f$?«Ç˜íbž¥?°Y¸Ù½C?Ÿeå'"è?¼ï@Ó?¥']¦~xd?ë*oñ·¯?©˜ƒ#sh&?fȚúöãm?Zkû^‡?ÂûÍÆF÷?©lª"¶AGN3FGL J1625.2-2845@uØ_ôö@,fÃb(À9xx·¡ÂÀ:ê$=Ìê)¿òôv	³@ÁþÙºF@)¾×ü¿êÔ½âvá¿é¬ë';¯·¿á»<QÈ}:¿ÓBBÏ»óUNASNone?ï'CŸ<ã?'£'.dŽÂ?H¿p6©@?GTϜ¢f)?Š#'&©oÍ?'p/ÙZ¦t?ï^Õ¨5?š*ˎ;ö?pßԐ·Z?xN™B0Ú?ïÑòlÎ?˜"ù^;_?ë{ÇU?­
××]n?¡†ãQë?"³"ÆmQ?¾'¡Ôô?©Æ£˜4?í÷ßèˆj?¡T_5—&þ?)¥ÕÑ
·4?.D¥æW#?°4-Òµ¿Ì?¡NTˆÙ³?ï׸WíH?xµ'þ²¾}?6"–˸¼?2ÏF}¡¼W?r»Š›í?xWô,;?ïÓt<¤k?uð¢d¡D?Yæ`q¯Å«?Uð§©?o˜"6_Ö?scgpä?î#½Šm4i?ž £á\Ù?Ï›Ï¢ì´?ƒŽw³ˆ²?¦P@få;?›ÎÃÙr~?ïhžqðˆ>?§Â–Xí?¨V4¶"'?Ëó·*
?'Ó‰nBÀ?"åpÙ¯AGN3FGL J1625.6-2058@v:®záH@3I§;BÌ-À9EÓ)Þ À;"Pg÷`?ÓXŽ-ø@
g%Pq‡'@SÏÿ²'Z¿âž¥ñQø¿ìáWb+]¿âøLòì¿ç¿ˆOªUNASNone?íèuQ槔?¯@†N€o?t1lÂG¤	?r'̇¶Ï×?®ò}G"Ä<?®1âÕf"!?íöWºs{D?¶›^Áô…?ŸGvp¦""?¡ö+;©4¨? öÉ!Pðy?°Ø'	Ï®÷?ê¿j´²W^?ªÈm2+¢û?§5'¯!Š!?"K]¼í³W?¾iép4ú?¦ëÑGm?ãý°xü?³I_n R¹?°¤'/Tæ¾? f¸'nŒW?ÕÌáåQ9?²ˆ{ã³ë–?ï|»—<¿p?—lû8Âœ?^ˆÒ\è¾?_ÖژÍå?ŒÿÿÕâ<?–ƒ:*Êä'?ïB7d	-À?¢ú¦ÃV_?†Uòd†ÉP?ŽúžÚ/½±?‰4œb°?š–ÄDk~y?î<Ö>÷ž?•Œcñ¯Û?"˜¡Ã?…B½Ã.8Y?¢~ÖK…øC?fÍC´œ?êA&PF?¡­‹ùNß,?¦ÂEÉèÐ?ŠÔb]ç=œ?ÁJÖLGÚ?ŸI†ìËAGN3FGL J1626.2-4911@tër{²þÅ¿«Ýqà˜ÆÀ8|‡5DÀ9×ôm$Ɖ¿ðÞ	îkX@PæMÒEÞ@ÚÁ`ˆ¿ç%—=$¿é«´x÷¿âì7È]¿ß¡Ìts€'UNASNone?'ª{Ήc·?•+—™ `Ä?`9¡Ÿ=?d~‡8{Ä?ïZè0-?–Ë4yâ͞?ÍWa¿ýJ]?Ѷþ³""›?¨†t%o:?¦S-@ÙM´?ç!Ç8õP5?Ñh¡HSo­?Än¦Pâ½?­I¯Ì`ì)?²'å¹Pñ?¡¡*xÈî?è'&/Ã?²JXŒÆé?×D¨'(È?Ì֖!?E£ì—= ?E¦>݄?äXBÏ]uÒ?ÌØöÍb…?ŽÉ÷L«"è?'™wÐ<?r,4Qno?"+ü­"Å?ï`ËÊnM»?—qèɯ@]?Ö¶k'ÜLX?Õ¢ucŒõÐ?®üKçåR?¦
TT±D?ⵆZU??ÔYÌò?Êç3q†¼?¯@æá1D?´ÿ:.xY?¢è')|"ë?æ¦KóbQž?²BžÅ"W?Úm+bÀzÀ?É5YüÔ/?Go(çÁ?<]	(DX?âæ²ÔŸ?É4ôßš}OTHER3FGL J1626.2-2428c@vð†nD@0ä^	}À8Y
×ÊVÑÀ:]$
üB?õ¡¼Ö_@ÇWC]ͼ@3õ§:A?ïüçEا¿ç@Îk!P¿ã¬¡gT‰*¿çÒ^ö@ʲUNASNone ?Ó󁚧ê?È·²á`¤þ?ÄñÝ<lÔ?Â/]ÛÓOô?àÉø;\ï½?ΣÒýaÄ?ãÓ]m‡5?ÐóÖ''?Ï|)ºA7‹?ÈÐË Ç˜'?Á6`'\«Ÿ?ÂG" ¦
?Úè|‹kÙm?´z¦ì1?À†Ž†ãUó?§ñ÷욤Z?ÜÔ<0šÛ?³¹‰¼mà?¶-"3"{#?¤?îH¨?ѝWæé%?»ú~‰Ó1?äk¡¦O×Ñ?½Ž›8Ö
?àu!†Í?Ï£Þ/¡?Ä1m|@~†?Àç:ْ$}?Ôý5¤&»?ÍJÒeÓÄ?ç
Ù̀?ÐoßA՞"?É/(aÿ°?ȹ-!l?µQ€pÍ÷?¼jÁ»‡ç&?à‰{b](‹?µ[±LÃÆ÷?»~`BR?£§ À¿Î7?Ø
q3/=–?µ&_ãóãp?Âv'	…Ã?©î?0"ä?Õe00tg?¶8w×M?àÆ
Cƒk
?·Ñ2Å̓ÇMIXED3FGL J1627.8+3217@Jz©?)
»@EšÙ¾L×IÀ9ÆñÃ&ZÞÀ;ÐÈ1\™^?õc\†=Ç6@úË²@=?Ñ|4?ïߞÎ.C,¿àã­±K	¿âÎ"žv´N¿ì"äΏ£UNASNone?ÁMëíq?¼äl¼ðW?êÖ§O3?¿×Å#`,f?šÃ®|	?›­à¯tü?«Ztp¹RQ?¸òéøå[?ë¡ahó
?Å
"?µGº}å•
?¼Û݇–H?×díd
Û??¸Xk/†§æ?à¾5{ž>?¹ö̋Ł»?¼zž'ãÙ?£,ãŠiÕü?µ,f£«žÝ?©$'_g ?ëjêJܦ?³ÄêžLX?®øˆãë?§1ÛhaŒ?ΏÙýÔ,?Ų½ÞX¡"?çw¥gqíó?ÆziàeÓ;?œŒŠ‰Ó H?–z´ù‡Åü?Â@)êùÍP?Ćª¾&Ž?蝇G?ÉqÒ]ãé}?¶–ìAv§?¶Ræ‹?ãÅÌ]S\?²ÏõZ¼bg?Óéõ†C?_?±§‰ý\q!?²)É4äN¤?™Õôä0%?љ.Êó?³MJ»Ý8?åÜAE*è?´Ÿ±‡Ë0®?¥ruSÄAF?œ/#vU0"MIXED3FGL J1628.1-3344@u£"úÖËS@$¼[òoÅÀ9ÉÔQüLÀ;7ò<ÈÞ?¼Ií´ÎÔ9@Ùéù-}è@îÉÿ½åÔ¿ëõŸûø"U¿ãg€¯è»k¿à)«[I8¿ÓÌȝ4¦UNASNone?î¬b~
È?¨AÙvr[?g+Ǒt.?dêAßk?£Ç!Ïùöþ?§ÚE¦ëKD?îoÿ1N¿?¯¢4
½?ƒídçÊè?ö)½¿ù?¤³¬µî?«ƒ!økñ?ì]A¢óƝ?§+¶uÊî?›ÜÐ~qÅÌ?ˆmÔ7Ýä?¶¾Çér§?£íX£
?ìgiyHõ?©7í,=˓?x~A©Œ?{•ò+øX?½ó,Ð÷?¨Í¢&äy?ï—þÛ¬}f?'Ø8Ò¿Ð?UkÛE'U?VAY.`¹?‡Rͨ h?'Pçiy?ïŒ#‡C«¦?' kƒ§W?mFË º»¡?r"¯»m¡"?…¥kE.™'?‹}Ý

žD?îၱ©?Ž?¯mkhY?…Â06Š×?rûŸwñÕx?˜û©cý?Š3-P†…_?îÊå[äØ1?‰÷'Àˆûú?q>ÖßZ!?cí/6£?¡)օ`¼(?ˆß•¡žGAGN3FGL J1628.1-5740@tŒŠ\å´$À"yÔØ4	À9²¥ùú,À;#áâއ	¿ÚS'nGË
@×qýÉD@¶ RÛÅ¿å@+=U¿éÐb×CPë¿èV™µ{Õí¿Ô۝Fï UNASNone?ëMù<íF??»(túd?SóÜ«ô?'"OaòKR?À½œ{E?¹é¨G(ÕÚ?ìmC¿"ÍN?¾æÄ&­`B?•©Þ¯OÓ?£V+¨à?·+jW…Ϙ?¹ã3Äè"?ê‹Çsòk?¯zÌaÞe}?«ÏéTs?™ Á‡›?À¡ÖŽ€Œ?©ˆðÖ¡ ?éóï&£?³¶ýõ½?tuÐo?uÿñÌX?ǐ4F"Ë?²îv%¯¬?îz
Ԙ·á?¨"ºzƒ¸?z©•»Â§?€¦8!Ó9 ?¥	ïþ6CŒ?¦Þñ`¬j?îÞZ§%?¥î4æ™?~ºµmk?†A)Læ?œ†))û¨? ûnåºå?î>ÍÅ	"Ø?"49êó®'?•
¬è‹,4?ƒÐ7•Œ|w?¡ŒM;(<c?Œ_h‰?î"Šùî™?•I9"Ûò?_æ&«1'Þ?S4N~ü©ñ?¬à–µÍe?"Úb?Bé'AGN3FGL J1628.1+0254@1¥‹'¡¡@@t<òϕÕÀ:L(Àª'À;´Ì3?æ"ßÉ\]'@M÷Y¾7@ú'ßk5¿º["'0®¿ ÷?$‰ö¿êP*v˜…¿×b2¢ó9UNASNone?ïéllÝo?fh–T[E"?c5)Nû22?e;Wi%aÿ?:óP!@¬$?7Yëºô#?ïfÒ¶,¬?™lÖnÁf®?€j þ'?…æ›B¼?…á2p¦Â]?"=¼J´ß9?F"?"Åmï?™Ybƒ+'?•®­›çÏ?'<'C:?ó~ÕW'¶?햠û㐴?¦&û
…'?¥$ÿgŠ>?£3Mu®Ì¿?¡pðÞóí'?˜{È«ÞsF?ïù!ඟË?J¢û†2*?DÍƂô®ö?HHpz^€?*ªÛXåà±?$ÝÃH }?ïËïZýbÓ?|0z%Eï?g`¹$¡¾?kMýÖ±Z\?l¯ëäîÃI?u¶Îêþuð?ïQ¬>.[?ƒ¼ÛQm°†?Šœ,Œtá?€ ]²Q?!èWIÂ\?pkªÿ¶W?ïtÿç‰ð?'¬Ãÿ³þÄ?"–Ýjo?wŸ"PRü?{úßùà	J?v/[A3CAGN3FGL J1628.2-2431c@v(C€ˆQ@0ƒ	"ãÿïÀ8wÒ<çèÀ:dVè'?âöZ'@H÷¿>Ä·@ú`Ãd¿çp^{¥+¸¿åM#"qÑ¿è@Û¾hl6¿âUQ©üúMUNASNone0?á·v·'#?Ì,vR'ü?Æ/:©}?Ä·õ®8?эûµ¦ý?ɾ'…!‰à?ënìrY?ÊÓ£ý0þâ?´ïBù'áE?ÀÁÓä2?¯@»C"ï?½ëvtë(F?á8Wª7?´^€C%Q?Ã"ÜŒø?®ÃNýFÅÀ?ÔKÌã"/‹?³Û?ÐQF?Áø4»•å?³à÷ï«Ã?Á§Âý??´ˆa×Ä>?çÎÁˆdØ?¼®N¶¶#Ø?æÍ:^(\ô?Ì°þÙ›?Á¬¢ö9­¡?¸:³I?Ãs'$ޏ?ÄCúš6†?íH—ýüßS?Ç$B†sˆ?ª!²/Ò%ˆ?½»Rl)?¡TÍòóšD?¶}w<1?䜀Ñôe?µt&#l?»î1ò\v?¦¶eÉå?ϖç¿0?²Êt
ž;?Í¡Ã/{Sï?¸üIsW?ÀN¸¬¦´?¦š$ÆîBg?äƒán
¥?¼Oζ˝MIXED3FGL J1628.4-4546@uô!-w@kOÚ2æÝÀ8`É{ßtoÀ:aùӖª?ôxËéM!@ª˜zµ©@6 %#ü¿åî_ª¿é'*u°—¿ë9hÐ調îà#ñ÷©šUNASNone?ǎKVYlÈ?ÂyÝ´qG?ÓB;À0ÃS?Ê8õ…äÂ?à{OJQC%?ζ²±:Ÿ?·%bÞ± «?À•ŠUÙÑB?Ö­ÆȕŸ?Ã¥ÚAC[?áÄÒ@e\?ÈuS3ƒ»?âUŠe?¬iÖ®.p?ÒÔ1Bö¨F?µ'÷ó¯?á­dI"*D?¸h
…³Œ?´ßÎS¬ó?£ŠºÅ‡?Øú˜,\)w?·MLeP•?á—ðL-Ö?¸ÖXzù?Ë°ô³yG?Æ\ž©N?ِIþ?ʹ9V&Áú?Ù#i¼‡/_?ÍÕ§¼È?ΛøÊè­9?Íÿ­°ãôB?՚"Òp¶Þ?ÁDµD<?ÛnÈò†?ǂ|7š1U?ÖÖʗhfò?´pȂŒÎ	?ÎÛá/ãÐþ?°#åbî;?Ù»DÐ¥°?´èܺxè?Á1V?«šy]Kûû?Ù6–G³&?®
̜he?Þc°å¡Á?²U,Íh~OTHER3FGL J1628.7-8056@sm‡~äâmÀ5ŸVûW÷À9àÁ3;–¯À;'yLò÷Ú¿À¢XÕâ©@ÿ‡Š#@»ß"¥"¿àzò ­¿êððØg,+¿çúe:í<¿ïÿ€
HСUNASNone?îZÌ,œsÇ?§íÂã*aq?‰É¿ò?'t³.‹Æ­?£àÍqِ?¤W}Á&}?æ±O†?Ê0ºäS7q?‰(Ճ¢?Àå"^Ø?±šúEà?ÀìIñ û3?馘ðHÊ?©,B[͹º?¸ôDÜÌÚ?¡V¬ok:?¹Úÿé×?žqÔ4žbï?á2"˜½?º ¥ðr¡ç?Æ«C3Ë"m?¶!<˜e%Ä?ҍúF$?·uäzìÄà?î÷U×¢é¤?¨ÙòlrÍ?{¨£/—?ˆàŠ7ߑâ?š1á²?¦W¡QžÙ?í$¹*6?¹|:×úû?¥5…ðZ˝?ª"SË?¨~è~´.ÿ?¯ªïçµÚŽ?ìÖ²Ы?œô±¾	­¬?­:hcÊ2?"ÛLÊçwü?¥Z@¶{?Mj­M¥?ê°·!-»ê?¦šéDºŠ¤?«…µÔ;?—RES
?¼ñ?³IC?£ wÛãþÞAGN3FGL J1630.2-1052@ ¹™aÝ@8È!~|À9ºV4¿û-À;Y¦ùÔlÔ?òz(»
-@7î-ð~@a« §U?ïRÇ:f®5¿åIøopƒÔ¿å!'óˆß¿ïý…¿û‹°UNASNone?Փ}És@?È=nµë3ë?â\*4©La?ËúøE?¶ÒDb³èö?³cM䙰?¢1ã_²Ùa?­thK‡¬¡?ì:"âÇϧ?¿x¸´£Š?µ÷8ž;œ?»¦UÝà¤?Ü/±{$Ÿ?¶Š‡˜Ó/™?Ú«tà/¸?·¬¥'ðŸ?ÂI³I»WQ?§Í\bÙ?­mùºýQ?Ÿ+zØ
r¯?énÀe;n?¹ÚB:¾ì?Âé Ús²?´JŸBrbÀ?ޙ÷ÆS>Ÿ?Ëò°6>*ˆ?Üò2¥u4?ËÔ5ì»?±ÏX͈9?«õŠ8Ü*?·tÈ	ž®9?¹;Ø=?ê1$©ò?Â9bÚGÙ?¸&¾m<5?ºžEa\?䚺7b±•?³	cs³O$?ÑD§.­'u?°èåìb%?¶'ŒÇނ?ž" ™-²?ÅUÑ4?¨!–9?析P''?´…%
©æ¿?À0£ìƒÌS?©ÙA~"IgMIXED3FGL J1630.3-6126@tcGd­ÿ'À!Í_™Ã‹À8ÿXz™À;\l <K
?Í´#¼%hM@–)€Výh@I`p-:¿éÀGáɒ¿èTia¿æ¯tҏڿïÿϲUNASNone?ïØH×h?t7V4s?G¨²æ8Ó,?H·þ¥?q嚐oè?r¶õ»|š?èˆó+?É«áù7?°&gìSñ?­\¯UÕ?ǂ¬–"[?ăJ¯ž
9?í';a3w?ŸªßæOÃ?¤ÀЊ•?"P¾Â«Ó?¢+A¡?'UtA>i?ëûcn'?«§sA®0?§ÝÉã"š?œ£[™]þ?»i?õ
ˆª?¦ùLv"?ïïñ?\¦'.þ ?BW	AÁB4?Cƒ§ÎLý?X˜oÛ¬¤é?W:ÜéH?ìÅÄN'Îé?¹…uª!T?ž.3ƶE<?Ÿb=çá?²FP›Ñç?³6:Ä_˜?îÒË"BJ?Œ"§ˆ3…?•ëXŠÿÚ?ƒ¥ˆ|¿?v^WÙm¶?€e$Â	(ã?î¢)¥bG?Îà"Í(?ŒÍ!èOb¨?'H"³É£?T:X°4*?‹TƒƒæP˜AGN3FGL J1630.3-4346@u2SâÖ@	†×:ÇÀ9ˆ³c$"À:ˆpSO?ðrD˶ø$@
mœ@Ô@P`j£ã¿ëA2'^>¥¿æùdÌÍ…¿ë|[Ñjžã¿ÜœJ°jUNASNone?žü¢¾¶}Ž?§ÃÛ¸R5e?±ÏúÏã"T?¹+nˆ˜Ð?ìΏä 9?¾¿;®p°?âzÁ÷?ÖO¦0€ÑL?©B
³Ë2¿?¯,8é¼­×?×â<,£n|?ԇ
`V,?Ó|‹Ÿd?°âiwU?Ï[Õ}?µ
ÿªT-Ó?ÝbZUêuÞ?µm¿~¹!'?Ð;ÔÄ#A?Êtt"iå*?££Ú¾'›?¬4,õ"æ?æ±éןŽ¦?Ëj}n¸õ?"hM±å›ö?'¹R̟Ž"?§50ê)Ù?´‹ç›®gt?î;½+!Ê?¶+c¤øÅ?ê
ÞIØ)?ÏÔOO?Ÿ
!¯/áx?§¶Ÿ²äù|?Ãæâ¦íƒë?ËԀ{̐M?Ô§Y<Ԕ?±·Q)Å£?Ì~·çž›r?²ÄþP—6?ÝJÏ\9?´¾qSl?Ò «ebÊ?ÇÂ-~ø?±yÌw¬?­3]Ւ&?䀊-YÄ0?É—pÁÖqMIXED3FGL J1632.8+3838@NÞáG®{@EldE#öÀ9àõø?A^À;áý¶z?ð[(ã#%t@.£yè@žXߕ&m¿ï̦¨1@?çJ<M§í^¿åvzÊeX¿ïÿ—Ö²UNASNone?କ‹Ü±`?Ì´<ÙE?ÙÌ1m5c?Ëúróù¡?³k>ßC.ï?·ó€7?SÊ?³:"–jI§?Ãߓ>òÀ8?ëBu%F
¦?ʬ±ë0K^?²±Ò>‰z(?ºîOa'?àö@¨?³;_žÍb?ÒÒƒ,V?°àäý]Gá?ÊO‹› ¤³?¬'œµŽßÛ?¤+sϚ,?£v³r€'?íX¯
¼hô?³øöâž;?¦eããÙr'?¬Ê/÷Z
?܀D P<?ÍQC»&î=?Úë¥G;ˆ?͹¡ad
?Á(,0¬èx?Âó'?	*K?Ä$ûÃä?Ëhº^`2›?èw¼2±ê/?ΰÁ9¬Û&?³ú
IU
Â?´º£i!
?äùç®ê'•?°ú¡v
̒?Ë»™s®ùR?¬±©ÄP?À\ÇШhX?¥Ýy—A?À"ßCO"š?±¥û;KÓ?éÊzàEûb?·¤Ö.bxw?°"jw0ý¾?§f@`I?/MIXED3FGL J1635.3+4257@Pèñ€
|@E:ž¡@WÀ:O&ò³À;òøK֘(¿ò½Fâ½yô@-Yôèõ¢@U1\¼™¿êîÛü{Í¿àÏñ´&§x¿à$'rŒB!¿ïô'½ÌµUNASNone?ï›WˆÁÉÓ?'…Gª?†šL"Ùg<?¡Et#Ix?T~ŠÉÿ?Ræf)_¼?ïy¼Ç­9?Ž-¸Äã?ýCÜ$Ž?
or0K†?'3'#çi?"u#M¤?ìëja©Ê?£,všTï4?°.Òåt÷?žãßËȎü? íXA6`w?V"G†b–?ïw4KOùV?†‰zª$?o¬…;!æ?sޞYe'¬?ŠGË×À÷?'\Žc?ïϪslÅa?rÞìz‹87?uµOóªQŽ?r»Yîïó?C«³6ÕZ<?C¥ZpUY¬?ïÖeNž7?mˆøÉÂ6µ?cw!Ò¿&Z?[¥=ëÄv?f#ݛJJ†?eÛ9/8®?î[ß`'?"ÁTÐe(f?¢‰(2nÕ?'©€
Š4?Žã¯cñœ.?~÷EȔ_o?ïèí":¤?`sœãX²ý?@K48±`?C‡4˜éó7?bÿžš+-4?^`o­À¹AGN3FGL J1639.4-5146@tä
"M;À
ËšþôgÀ7ìú@£À:®ŽwýgŸ?ãÜzª@>`ÔV.
@ËBàO`¿àüöøoh¿äÏ>"¿äk°ã«á¿æÇ1'ý¦½UNASNone?èñú37dñ?ÀPòÖ÷ž?¸ë¼öú?µÏSÅyò4?¿…©¼¯ý?·r¯L×/?ÓGŒ§ÔÖî?ÑÆÉ}Œô?Åę¾hÂ?º>sX<W?àë<{d?θ/ò6â?â¸c °²?·±_­~l±?Àò.Jâ?©à½LÈ?Ò¶¼,?´,Ì£š?Ø|׌s?°ú~p½:/?»Z'Ìå,?¥Ã†bfCÚ?àV©:݇Á?±Ôé2Öcq?î/‹jÏ#6?°™p‡°N?ÕÜßÍ,/?¢3ã;f?œ8µÆNm?©ÐB›W *?áB+$,@a?Óp¤sÎj?ÀTá%@Ï?¸ð4
<§£?Õ:ÿH'¿•?Îð°úð]?é•ÜÇÛe0?®xšx?@ƒ?³îeZ¿?¡ŸÇó("?¿b´¢€ëD?¦â+Wí]Ù?ãXubÓ?©»%{~é?³"VÖ¥?–•-ޑnž?Ô LñË3ð?¨±)³KªMIXED3FGL J1640.6-4917@uÕ<ÝÖà¿ýX™¤T(À8Y'£Ü»À:aÙïÊþ–?ìüÞ8¿_@A9ˆâ½$@tÿÑ¿äÞ~r
l¿ç~%q ù'¿ã0¥c@0¿é›XL-'DUNASNone?äpm?Àט?ʁîs ð!?²ÎËfC¡ƒ?³&iìWׂ?Òkr§åN?Ç´Õ·N'¼?Ó3GÕy?Т_$lŠ²?¾`g&ˆ^?´ӘhÎ?â£dqwD8?Ð
wÈõŽ?Úo4Iø`h?¶:ÜuNp,?Èc{$Ž€?¯FBûðTP?ي™øuXX?µaÕ¨«"Ë?×onõx‰÷?¾ã73?ªnÆ#"Ã?˜I… Œ~³?⨘ÓÃX?¾1P@E{›?êûQ}~¹w?ÔÆsõά?«ïf×"Ý?±Ð65Ê{à?º-ìaè}W?¼Üu-ËâŽ?àz×uƒuý?҂d{L?·ðڕò¡ò?«xL)Ç7?Ùo—èj?Ð_~JˆºN?ãü3#÷_?ºGpàpv?¾ã!YäDZ?¨#UŸy?ÐN5C?,?µ桳d?àhìùw·?¹[™=È]?²7‰ç€?"ŠÖ†¤?Ú EÜT³?·¼‰Ò‰÷¦MIXED3FGL J1641.5-2856@uü«¾Ê«Š@&ÄÝÛ
À9™­»ŽÀ;6Õü÷7?먕_ùõ@tî¹[¬@] A"ô¿âH`q"Ó¿æ´æB®j%¿ëU¿]´¢E¿ÜhW΄C,UNASNone?ëõ.°—Œú?¸ù‰pyI?´-i¹O?³l	€(Ѩ?¨Rêï³½Ã?§TŽÝ¹?í_ó§i³?À
°·îCj?™¹ñ&>Q?§*i¨=µé?­#ÖOÖ¢§?·Ì'À¤"á?ël=±Í~4?¦óȯÉÁ1?°BÔ¹³Èø?šP!à¸W™?´[=·rQê?ÜØUkJ?æ \|Ù?¸»ü
ƒ?´Ï)nD?±Ï§ø4?Ë}")Ñ¥?´7¾‰óFO?îǾj´SÚ?£ü…ÊuR¿?•à™ûl²?˜O1d¨«m?''˜§)šÆ?—:í_ì1?ïá5u¾Ú?¨á³€è5?"žÿŠ}Ö?•¹‰.7W?'ôYÃ:³Í? D`•ÔÚ?îA@X?•~@1OV ?œ` ìT-?ŒvŽµaŒ'?›·Õ ¯-?‰5O8zÚ?ìgùm¤?¢Uzk
l?¦ñ"¨)YŠ?˜³Ÿ7öB?±Gma^=?™=/Êî²BAGN3FGL J1642.4+8045@\oÁ½¥@?ÁP¹U÷ƒÀ:A)Ý:ÙÀ<u^Pî/?ÜíÔ¤v[@j×9bL@áz AÙ¿ÞÎÕù#ö¿åÐ×b¿é÷Ös¿åSCTF0ïUNASNone?ïÓ±-K?qõÊqN´?gIµU9©?húÿѹ?e| Ôó?cu^ÜÆH[?îdOèBœ?®kዲ?›rëz¤ñB?¡èP[u?˜}[K?¤Ê˜dò:H?í×|!'‡?–Ó£6Îõ?œ%Ÿt*ó?‹²"æw/ò?¤{¿oY?¸gGßS?ë¾Ã$,…?­*F)Îé?µê?Qä?¦·Äe£‡?©çù;$J5?¡ Íž"‰?ïòg~X9?Vh|·$à°?Gë)Š…P??Hwò3M²?O§9
|̀?LÑÙl'zq?ï‰;ÔÊü?'×w†Ûb"?ˆ¼·¶Ò?†Þ‹sã'ç?{í%wPËø?†~Ç\¶Í?ï$Öòü†?"Nf†`D?‰äÞ;ŠÊ?|æ
übL?Œåe¾ ª?v'ñ¿Û?ïÎMˆýs?Š™ï™q?"ü1>fm?~VàߒC?T
.²9?¥[Ï š÷AGN3FGL J1644.4+2632@G;Ž!–R½@C@oiDg8À:*=h@[:À;¯³æKùÔ?Þr[…?x@
÷û%$ҝ@–ˆÌB¿èmsZ›Z¿î¡·ú~a?Ò½š¡Ä4¿ê,9ÓÐUNASNone?ïdæ®í‹?²0^Œ Œ?ƒª,Ñ$¹^?«"£
'T?ƒQ~¨eÞ? [9'–ò«?î‰4«¥µ?ª•U£[Ëi?œjOc?¥/¡_4
¼?'o–´aò?"¯8éàÁ½?íK`6?Ÿ$yÙ¹.?žëŸì\·?xΜ%}?«Ô/qÁá?˜¡*A#	?í[V"ª¤?³ú\»Jvú?É¾ê$æ-?¡·¬ŸÈÂ-?°òß/¸ÅÓ?±
ˌM.F?íT£vDÞ_?ÏO¨šú}ñ?¥-="R²?«QE¢e?¥ˆ‹ªêö?Â\DÚ$¤$?ïG$4ùÃ?¡CӄðìÇ?"Mú.¼?œ8† ™g@?€²ßqÝ@w?"ÈÌÚ["2?î³eà¦?'?«š]£?Á[pY?…,rIª‹2?™‹sÞó?‹¿Ë±Lè?ï)ã­Œ?—*`Œî̍?(šÇÏ´t?=á\ÝÃÃ?ˆ^£me°Ÿ?‡Ôxå/tVAGN3FGL J1644.6-0911@!ZWɱh@6ßpyåŸ,À9¢{…²\À;5£"ŸY¿ÕÑÝHו@
5ré×u@‹³ŸÕý¿äÈ^gƒ5Ä¿ì{"'È¿Úqì"õÆ¿Ùp9Ðþ'UNASNone?ï=í˜Á¤È?šþ"ƒôÛ?[?ñË#(?\"‹ø"9?–ŽMÓJÿÓ?š$鞏"?ï…ÎOü%?"hêÀ¡Çñ?x€Ú•Á(?€±$y«Ã`?''«–qF?2B<éÜ?샜=t?¦+HÂêà?ž)®7&?‹ŠAFx2·?·éw'­w?£L[-@†?ì)ñ¾Ò@Þ?§ËT—dÆ?g6œÙ›æq?i­íÓE?½ö½ ²R"?§ªj/`.?ïÂ׍ðîë? |v'š!õ?H¶é?Xd?IŒtIh?{}[ïk½{? s²ra$?ïÔð˜ü?uÑ£÷sá?bƒH­5?atl@Ìu"?h÷zd8þh?p9µq$$3?îÂUs²æ?»NnNÇv?‡fgtºð?xNü O;_?œé)a¿?Š0
÷ªêü?îò¶/¹g?‡ç<a?\Ú?¸ñ€?N{û&T€?ŸÛ™äÛõ?‡xv­]%2AGN3FGL J1646.9-1332@ÏV!tÄÎ@3ä_ö"FÀ9ý»´v"²À;R]¤öÄî¿ó²¼ökÕ@
äË+­-?ý›ÃNúº¿îå±ç‡ýÕ?ÜŸŽ%G7¿áJé&¿Õä£ÖçáYUNASNone?ïx~?ZœLOWŒÊ?@&çè ô†?;öv?}?Z'ƒ~"Õ9?VLAC9	?Ö*æÖ?‹§Œ.?p»‹  5?w±¯¢ˆî3?}ò‰Í,CÚ?†müs2Ɗ?îËQuZ?Œ± å|í?‹fHPª&*?{"D1ë"þ?˜âºÊÁ¯¸?…ricwÇØ?ï@¿n¤?ïº$Ž?S}™CÂ|Y?W÷2]Á˜c?–°8ª\·?¼?ɵl?ïù{+oo?EÄ}5ÚñÒ?,r"8/f?%Þ0Í@Á$?DyqâçÕ®?B˜ÈCU¤—?ïÞ咅B?lr¿vF]?Y-pµLŽ?RãîÊÔ÷?dƒµºS˜?gJš™gÓ?ï}ž"©·?uõÌg¥•K?|{ñõE¨?o…¯(3&?'Éç:Ç\?iISÜ¥È?ïÊÙ[a¶º?jiµ».,?,¡²Տu?%¸Âr>]Q?y®D±•ÐÁ?j¡—hAGN3FGL J1648.0+4230@PÄ:}ªOÊ@D÷œ"/¥À:kªKÀ;òÛé B*¿Ô\È/%©Õ@|s(@»Ý@×mŠNοàC±‰`¢"¿éæï'7ñ¿âŠ
î¥H¿ïç»ÊŠÁÿUNASNone?ïð奃)7?V›±üƒË?FOdS?DP¶¶ex?S4¥ü	ð?QTÐu¦…È?îËÑü׸?¦b'þ<3÷?"Ão=ëìú?"¯æfÿO?'ÂQ9Q²? TMn¤¢?î?]ãàæ?•¢p72Œ¾?ž4X䜖?ˆÎ"âÈ?ž¼'W¶?‹zAQ¾k?î0·©–´?š.e¯auô?""Ï¡ØN?Š
CÙåQ?¢²&'æÒ?"a.»v±?ï÷m	˜?Fª1á÷g??<i‡jz?9˜Â¿¡]r?B«ŽÕ}'‰?=%ՈȈ2?﬒t°£?¾Uß²7?uTB¸Ã'?r0¡ï7µ–?tbºÖœV¨?tµ"ßi1E?î넬çC
?…>bŠr?"¤b»Û¹?~:íU?‹Ö\7?uà»-Fkë?ï¤XνÁ?t
Èû9ý<?rãLþ!äÅ?bsL^	?zðKªìÞÖ?pk4´ñŒAGN3FGL J1648.6-5635@t·k¤"ÈŸÀùõß덂À9CCÁð`À:ýàl¼Á½?ôSÈ)$@
)œ–¤Ô@hž\‹¿ãžõ"YŸ¿î‡Ú%—¿äJÅk¿ÐŠÙD¶UNASNone?Ëú)YôÍ?É
'‡#?˜…FÙõ?›¿]õêØ?èAؽ?Ê_dߨœ—?æÌ·PŽ¸À?Ðbz³ûD¯?¯%HCM£?´	Ú7ÆG?ÍЫ9æ<?Êð/+Öae?ãN>žÃœo?²F 5ȗg?¿ØÃcäÎ?£ÔXõI«?Ñm~Ò²®­?°â`âtÓ?àÅ×nÖ\?ÂþôZc‰?´¡ H£F'?º°š¸¹«™?ÙL	}"C?Â[3u€é'?Òg'WÓH?Ìå=֜§?ž­ÞTqŒÙ?¡©'œ:­?åÖÇá;ÕÕ?΢>nO¾Ú?ì€uþG5?Â؁DýϾ?œ´¬¼Ù\?¦ý¤Ê#?´Ï$ڙ­Õ?½-hrI}?èÞ=®Èf?«2"?µœ¢±/a?ž)
qÌ?Á¸·êÆ¢?¦A#º.	Š?èsò¸f0?¶Nu;?¶™ÿmyy??±è &¡`?Äi0}Ð#?²YÏ#³GMIXED3FGL J1649.6-3007@vð¹@"Šl~®[ÈÀ9
д¸ÙÑÀ;!Š{¥?òEaƒ¨–@¸¦Í^Ã@"É﷿ߟ-ý¿3¿äõ힇¿â˜µ˜þ"¿ïÿôo±œMUNASNone?Ò~GÛ®3|?ʤzóJ?ÚÀ§Þ^x9?Î`¢|Q?ÒÁEóTK?ʺM'>'?Î(7ªn܊?ÃÙ#tp·›?ߝq°F"I?Äé4Cuíå?ÑNryo,´?ÅRc"çî?ÚÊAuHßö?µ!"©‰•"?Ø-ŽGoÅ?´Èu>w]O?ÊI!øß`‰?®ÃøGé'?Õ¾yÝç|Q?²Ï›‰3?ÙOehcI?ºD†¬×?Ðò!!° f?±Á{œï¿Š?ß؀ñ=V?ЧºÞQžG?Õ'wò'?Í7é³.ãe?Ç®ç¡?Ņ¹¡æˆú?×Öq€¥?ÆY>B(«?ÛUñ¨h-U?Ã'""ų9?ɨÏ0eŠ?¿åÃ0õHõ?å<$•Øç?²35ƒ
?Ëj²?F«¥?¬&*¼Ìb?ÀL].að¾?§8ív)kÎ?à៶ØÞm?­êŧ?Õæ2',™?°áD;ä?À­DQ?Ÿ§†`©NMIXED3FGL J1650.0-4438c@uMIº^¿–ˆë¡y6ùÀ7P+ÃÓ)À:
™Îr¿:¿´ñ{Nr,W@Lóin¯@«"¬î‹¿åU5_™~Ó¿ç²¹'[ÿ¿å™»µÎ- ¿ë	—B¯0UNASNone$?¤å½r\€ï?£uc‹îö?¸¡Ô¬ L)?º¶Èéé=F?ëi"4¬?¿X¦ã?£·UT5Û?±Ph)?¿¤CÒÎÖ?¶+.LJ¡F?êäP'x?¿È™†ŸR?Â#à§AšL?¨©N†!¤?Ði÷YW#?²\ȯÿ"?ãB)"â?µ"ü«P?Çì²»~›¼?¹Õçä?¨B-¼š³G?¢ßY-£S?耰udlL?½3Ó+¶'#?ª<´¦»@2?®B@ ÷4?ÁyÁ[™G©?·¶Ì@œ?éýÄ^iAã?Äí"Øê'[?¸ö¢ß ?Ē ðP
?ÙS£–?µ>'ºfʎ?è'ZÖÿðU?ȤÆlûÖ?ǀ9£\2}?®P¢U'H?ÑÜöÛ¿?²~&çïiº?á1v)Òâ;?´óòÏ)™8?Ñc_Ä>fv?¾}!Wˆ?™‡šš¼?¾``X~s?æ'a<þ0?¿"¢ÓeS}OTHER3FGL J1650.0+0356@5Û;BÌ-k@<®ð®SeÀ:)CæÝõÀ;•ÙÔóü¿ÕøD¸0@[ÛB±Ux@S€?ÖY¾¿é¹€á¿â6 $š‹~¿Ý["¾¿ÖLn£UNASNone?ïþn.©-?,š¨¡»E?îÁŠP?[‰râ›?'òêRÃî?'Á™Bœ0?ï¶D 
é?ƒZޟê_ê?nµ0nGßO?w´ÔÇԊ?uƒÀD·î?y?.p®!g?ï~u¦AÀ?~29ªšï—?v»#ÄÅ¥?g󟱣?…éÍ"X?xãëûMØ?ï·e›Î?uª}âó?*8‡šH?/—¾í\'?ÓD‰gŠb?tâZï·øÈ?ïÿ`ç\¬:?éڀ"Å@>úH£¾*Û´>ö¼RšHj?
¡äÏqž?
€vQ¿È?ï䃝â\4?fŽ_øbУ?Wqœ_Ë?SÑÉd¯?_‡(F#߆?`‡‹Pˆà
?﯁Q=#?f•›À2Þ?i3Pr‡Õ?V_¦œÖ?r$% ¹ÎŒ?aòŒ©°­?ïò8ÔTM?K÷N²õ¥Ü?5À—Z«e?ÞNJU¹*?YÚûsß6æ?K·E
,ÓAGN3FGL J1651.5-4626@u9²þÅm]¿ö~'MKãÀ8ÿÔqܼÀ:2¯È¿ÿÛÂMíɝ@
dy¤†²Œ?þ¿+ie?ç"LšÀÇ¿ãi‹™Ì<¿àŒŒ¾¿Ä¿ãì·£2UNASNone?|yãÒÈC?zÐì#üŸÓ?h^<Qt§?kÜ
÷(Z?ï®®lö‰›?5.øž\V?ݣٚK×U?ÖleǍ¦O?£çŒì?¢¡ÿû•Š?ßûË?ՓÐö¹A?È~ÆS$Ùî?¬Z酕+?®™¹a€?›1Í^keí?çö¼ß¼5?¯SMcmà?Þý(aÈó?Ì»¬Ö"¨é?AÇú«|›)?L×pŒI»?à}í@Eü?̽ %
6Ì?u³kÛa5?|Zìöèô?g¤a,@~ä?t}n_k	ã?ï¼õh;AŽ?"µ ú¸Ã?å`Š|EJã?ÖulÇ15?¡C*.¬Û?£X«vgš¬?ÓˆÁ¡ ?ÔW°3á?Ïi*P‹ˆµ?°%è~cp-?±÷$|ã1?¡SŒ ?åæÐèv‡­?±Ã埣ì%?áö)ì§Ly?Æÿn™ªzV?/~•rhÙ{?3"ôZdí?ܼS¶i?Æÿ3¶>ìMIXED3FGL J1652.2-4649@u5ö_Ø­¬¿ûàÛwŠ{À8¹°,À:=yaë­c?™g¾yNªÆ@ët±­·‰@»ÍŸ°‰ö¿êí\Ò
q¿æÝËu'[ë¿Ö‰óü3B¿ãክ~ºUNASNone?ÅMcÀÄ«Á?Àå>¤'«u?'Ñ6ëƒÚ?•µÀ<Š?êXÅ,ß?Á³<^fMù?Öþøïüì?Ôs¦Ðä´u?­µtJèw?ªø[öÔH?⦨0"Ï3?Ó³bûDPß?Ò»ÀÇ?²JAÁ«"?ÂeFú•?²Žƒ†lG?â\'¡?·kTÒÌ2w?á1•lõ\õ?ÇúJS5\?jŽ¶WÉ?i]sÔ³(?Ýg·ºã?Çú'42È?ēó<x+`?Á˜Åßۃ?‰/MOŠ?F:›8ñ?êvG$à<Ê?Â*µԟ»?ãB!wë?ÕÂzØ}ý?¨NÊö*`ž?¦¯fO3Q¹?Öq㲗ln?Ó¼廙ˆ?×%^àFbv?µÜöN Ï?Áoú‡Lª?®fî{1õ?àR
úûš?¶Eî»xÖD?å:§TÜêì?À5'À&K?zݙ 'î˜?iiCdRî?Õ:ïPkŽ?Àõ>IÖ}MIXED3FGL J1654.0-4617@u?ž£Y5ü¿ùҌDF€îÀ8Ձ×ÛôˆÀ:a6=©®»?íÖ¯Ÿ?uâ@[ã‹U38@Ÿø-y?åÅ°óADˆ¿è6
g¾øp?Öñ\Û¿âSY<÷UNASNone?׎j@æz?ÉÝ­1saï?˜‹¿¼C?—ã`>Ž?ãx†ŽàÙ?ÊU×ÿ¶Q?Ê	k°"?ι#UMB?³Î$XØfç?«©\"'®?çô™øí›?ÎG¤¯L^R?Ô@ldµ¿É?¹ã›2‰?³Ciœ‡ÒË?ŸÛ[çϋ?ãw\š'B?»L:ZÍ?Û8*`H7?Ç`±:õõ:?Œý|ñVê©?"WÏt-?âm÷>ª?Ç£˜…Ð?â·"ÿ£Ë?Î KÉpæŒ?œ´Ò­ð?š}vlP³?ØÆzK(P	?Í­ÙéQ#?ÛÛBð¯Cê?Ôñù.L?µ)[
Ù?¬ï2'}+!?ÞÚfL~ør?ӉϻÙN?ánU'¾3?»\ŒÀ9¸Ö?°Ì%§xb?¿T¿?Øð1Pó@?ºIˆ×vì=?á÷'Ü4k9?¤Î+¸?¥öo{˜Š?˜r/õL?ÙRâf£3]?ÂPÙ>þ¡MIXED3FGL J1655.1-4644@u<`ÔV.ÀO¼ä!}(À9GeÆ-vÀ:jÏЍK­¿ö'kØ@
«Ñ?þäw¡!MX?ïýt&Ù?¼ú]‹˜ÇY¿ìDñ/
¿Í)ȃðnUNASNone?Îؘ}9ç'?ÈòåUH¡?¬RS¯ƒ?¯B(H½kØ?愴¯
÷?ËHt´™
?â
Ì2Æb?Ö§???¢<Í¢Ë÷"?£A:™ð0É?Ù¢ÎG\q+?Õ5^( Ó?Õݪ]¿¬[?¶ûŠÉáÏ­?Àz¢FŽ§?©|«ìë@Ï?àò'IN†)?¸@›î¶ì?æþŒJ²›?ÅU8Æ?s ~$õ$?"åòdHÝ?Ñ´eʁ[?Åùítë˜?×Oá±­®ò?Ж¡mE?&•zúŒ?¢JŠJ˜Á?ãnÚ{¢?Пpü Æ?èA'hfµ…?Ó$^ÐV*j?›î›ñ¼#?¡´@ÄÖû?Ë{âà›œå?Ñq8«åT?á[2‹ö÷K?¹îDgt>§?¸eÔŠ'?££ÛÜü?×0%åËT?¸Ãy0h^«?êÆW"ß?¶&yj¥x??Kñ6¸ž?AWìÜ>J¨?ÄØ@«8Ië?¶"Ÿøì+MIXED3FGL J1655.5-4748@u/€IQƒÀ1Ÿ<pɗÀ9	ñ}†=œÀ:v¦ ™@¿÷ú­¥ë§@'6µð@ü½¿h¶"¿äBVãVž¿ë}»Áãe¿çìѓ'¿Ñfn`¨-ÓUNASNone?ɊuschÊ?Âòâ9ŠT?Ž:5:\bÑ?"!aéBèø?é$yÎfï'?Ããˆüq?å'öð6ß:?Òå¬ïî?ž]r‡Ò'?¡"ÐL­/?Ó:ÿGƒ?ÑÙ`Þ+Ú?×sCÛ[?¸öZ ¦ß?¿pbW|Ø]?¨/ñ˜àÁ^?àXR&"g¦?ºËÚkhPC?éGÚ¥ ?ÀϹWf?/K¡q7®(?5eÙîðàý?ËÇҀÀÛ?ÀÎRܤcÖ?×dn‡¥®Ù?ËåTáŒU?v¿µ{ç?Ž0™ÁUÌð?ã×î…s
Ó?Ì?Åt¶,Å?êaä2$ü?Í,zDÈ9ž?–0ïOóL? '?'¹œ?æÉÐ:Œæ?Ê8µüÚ9P?åJlÍޚ«?¶`a*"'^?´‡šIá?¡½uF&Ï?ÐI?Àp"3?³»!¸8J‡?ìÕ9oý?ª×#ÔÆR?<ÿÜ˂d?ÐL†Çí?¹PGÇéû?ªÔщ70JMIXED3FGL J1655.7-4712@u7P›ùÆ*Àhñ[!ŽÆÀ8ìùTëàÀ:O7iù˜Þ?ã·Ñ$m@
ñk?¦@ൟ´Á?ïÿÂ8&ì¿êú(­Âý¿É
~XJ™×¿ècÃ`\UNASNone?¼%£N_o¸?ÃÎþ~(W–?®¼B܋–(?·bšcâá3?ꏇhÙL&?Éç"Û6?Ò"æAŠm?Ñ]7xŒ?»ßýk¦U?³r<ØÂ\-?ãrLjwÿ?д¦Ž'S4?Ðp€Ö1Ù?²äÓ(Üm)?½#è×3G?§tÓØØêU?ä%øBz«?µ9‡$}áù?Ïm(['¡t?"È1» ?™ýß}ú8?™¯/ñ?ç\¥ú>ä±?ÃwñØcȖ?½ìD®¨?Èwev@<ö?¦àš+‡9½?´ns/øk6?êÔmÇr‰¤?ÍE£š›Ä?à¼Bˆ](œ?Óöpt².'?¹òÒ§œ?³Që‰ZÚ?Ø
úº›ÇÇ?Ñg8MÏ@Å?×ƽl.?¶ÈE.w?½,÷"ÜH@?§"Š¥}+?àwŽáÀá?¶*•Îàƒ?Õåè0oMZ?ÂI†Ô?« !x>¸Ê?›k¢ª(Kè?ãS	Жäf?œ½ê ŒMIXED3FGL J1656.9-3919c@u›ñ©ûçm@«€>~ÀÐÀ8ÙZo¸ÀÀ9o+-«3ö?îuƒ2Wž«@
pµÕduö@ŸÁàŠ™Ì¿ìzÛd%¨¿ä>lbm¢¿â~­®Ñ¿é¶Z'àùUNASNone)?™éðk"Õµ?¢ð7 [H?Ì	5ƒQ?ÌÐ,™¢97?è.c<‡½?Íú®«éA;?Ýÿ»Pge?Öÿêé9âF?µâïÙI7?¶¨ Í@jG?ÝtD']_N?ÔÊx9-@?ʏ,>ˆ?®lfہE?ѐ9Áö7³?³ÏÕeX½?à"bÀâ?´ÚØl"Þ?¸âóÀè¤?ÀÙ
ê8? án"<?¦l ±½ö?ëÕ¯Îý?ÃtºFã>S?xÑW…÷|?'Ò&¦ßˆ?Çgwo3{?ËnS/Qý#?éôœ4(¦'?ËÜۺȵ³?åUE‰Ìòâ?ÕkX*ZéÓ?²B"Nqm¥?·H†œÍ3?ÐÄìX®Aò?ÑÉ}d&<¢?Ѝg(¦?°(4zØz?Î÷‹‰­à›?±O1÷"?àVàó‡?³˜æµ'%?³G½9B?¿Òä9·?±Ä6vÃ?§»áò<·°?ëvÏÑÓ¶?Ãh«SðMIXED3FGL J1657.6-4653@u>tSŽóMÀÙï_žÌ	À9à>™˜ÃÀ:zBf¬ÝC?Ò©BeøyÆ@!ЂŽæ@i=@}H«¿íޛ›^?ïý°X瑎¿ã¯ÉÈ4¿à"‹Y"‰UNASNone?èg¡‰ýð0?æ''¿Zž?Œ™Ï÷?Sǎ…¥'?ÌOæŸS9Z?Ã[>ÄO¿u?äXTښ7F?ÓفęU?¬é
~µÇà?¯jaõGÓ?Ó²4ú¢aÙ?ÑàÖïæ?ߜ
º:›T?ºdAëTCÆ?¾Æé&'d¦?©?ÝF´È´?ز:ü;‹ƒ?¸µ"à)ÿ`?æ¿ÃÞÖSx?ŖØ&Э?´Lú]z?±GÂ{)ö?ÊÚsU¯Z?ÄîÁzo?ëi]
êa*?Àt—‰?†‰Ò$ï?‹þfäÛè?Àñî±ñKª?¿ÎǛ,
G?ê¼SÛ?ʔé[£¿¸?Ÿ^¶›.?¤VE«âšµ?Á$/…/?ÆÖSBaX?ç¹Ü/ʕ?µ$fÍД?±Fà7s? Î¸¨[1?Èuž£;%?±û§þ§"?ꈢ'€dƒ?µš6zŒúT?ŸS{À$N½?'1ätKf?Áó>ÕË?´ŠoÃd÷¯AGN3FGL J1659.0-0142@1¥Åo@7èSŸºEÀ9E¦N³Â:À;9ÏÆl`?ç2ˆ?¡x@$'RxGå@Ž™`cÂó¿Ùœ{©Í!¿ä𫲱ÿ¨¿Úþ£ûXŒš¿ëÃy¸sUNASNone?ï-MÂíI?™XŒ·?–DŠ"ÍG?—á±%ö`y?pFöƒ²V?ooN3#°?íRL%ûð¯?¯ª×Æ°;?¨p‡¿^?œêмóQ?¢j¶ŠÉ¥¯?©{YÌ%è/?êèð¼7¡?¬íSí©@?Á gš-ï?¨ÖþGüÀq?ªÒg84?—«¸ÉîG²?çND æ6x?¬'ÓC3†j?µOo[å?£Ú£'­è?È5û9œ¯?§5F/zœ?ï¶C¸*m+?€@¨"+ ?~­Çî}‹ñ?|ø°)Øf?XÁpê*}?W/™­ÛD?îÊȌ\€p?›KAÚ±`?–¢ÿ­T?ŒsK¸T?ïg›3'?"cÜ¥0F\?ìø´	Žå?£~íÅ披?²& ә¡{? ôX!Â,?˜Pûˆ0—v?Šì¬*Î[?ëæ®%Joî?–jÏÂû‡?°}G‰+M?‹]'‰2?°MGMÊÍ¿?Ž`ŸÞõFÓAGN3FGL J1700.4-4019c@u•ê~ùÛ#?ó/ˆƒÇ À82NÛËÀ8—"€ãÀ?òw"pèu@Ò]×K«Ð@'¯ŸëBY¿áÔ.LæÚâ¿Ü|ùÁm¿ëå¥:%"Ž¿å&"g3HŠUNASNone$?y«™Õ3c?"cÎzܞ?Ë]¢c}äî?Ð<¿ÿ3ý3?èö~ê®?ÐY"¹?ÚáØMŖß?Öc¾ôÐ'?µò˜ìÔÛ?»""íw+?ß¡wgj?Ô¢"•·ø?Á´éì˜D/?¨2-\ ¬?Ð/pš5 ?²|,C9l‡?ã{
wŒÔd?´{{TÙ?ª=Sçk†!?º‡_QÁ‹?–•½BËi'?£ØXàۑP?í§|×I±?¿B¡e?ö?a…ìèoñM?q£ªD,ÄË?ËÍíuܘ?ÑÈݒJx}?èúþµ–ê?Ñ×±Cü¦|?á\ñÛ	À?ÕSó:u?µšC=»y?¹ùy(4ýc?×ߍI¸?Òm¤(îš?É6™±¹ÃR?¬/–l?ÐM¶õ¨–À?±Þi!¬£?á‹~F´+?³¶ËهÆ2?Ÿ^ö§Þù?¸\œ_̸?›ôñ"$j?¡äœÍ*Àž?î,È£z4?½›°âÐMIXED3FGL J1701.1-4930@u# ¥&•–À42ðîÀ9peÓÀ:«Wãä?퇩Þúæ@'$«@'ÛŸx€Å?¿hf±9ôC¿ì+4>ԅ¿èóO™'¿ÌŒ–"w8UNASNone?â͹Êo-?È(âÐÍÁ?ÁiDŵ_?¿p—Ø#m?ÑäWÉÑ«ë?Çù×òůÍ?ãx!rÌ7?Ò¸¤'M]?¬?ÒVc3ã?­•ŽWe$?Շæ»ô–?Ðér`€Úl?àÀ•
½x?¹è¦#A?á‹ç"?°àÔ8‹h¨?ԝ…þ¼Î?¶&B/H™¬?à‹D¢ã+?ÂO|"¡Á?ŸhÎÕÎo?¤œÐP|ÿŒ?Üøi^éD?ÂWóºö¹?æÚQ ȼ6?Ç]'~u¯b?´k°Þ´Ê°?´¨Œ0~?Ê`ã~?Å»¦+4?êæ±hÌ?Ë?н¾›? &«NB›@?¤zLÇl?ƽ (áÃ?Ç´–ð,Š?è²ðÛ}r?±Põ¼µF?·¶¬Ä¬ˆX?¦\lƏ?Á\UÛ­
?©#6ϕ—?ççd`&Ü8?´÷ôUU[¢?Ð™=±Äç?–ç̝öø$?̨[W®V"?´§²ÕÎÖAGN3FGL J1701.3-5216@ublvKÀüÂ]ÞÀ9‹i"ÙHÜÀ:öÔ2ò›"¿æzB÷ÔëÞ@4Èaƒ(@Ó«@`m¿á|_)¹À¿é|Ρ}¢¿ë—¨ÁæÐë¿Ïß:sCoUNASNone?åÙÿ1‰?Égw9¼.?•¶Œ]_ÆS?šÑXüB¼?Òð™!ÆñŽ?ÉzƒÁ?ížU¾Öóu?·ŸÑ—õ­?Š€Ö;KÇ?™óÍT¢'¾?¯znŽ±'¼?³x^ÔQM?æÇ1€¼º?´²ìßüOR?¶â˜—w;²?¤ÊÄ%\¦Œ?Éqí°>™?°®*ù'xt?êP m
?¶é.¶¯{š?bª{@Ì?hº"‰[Ź?ÆrÔ]å¹X?¶Öî"?êÒm¸À%u?Á"cþ	ä?}º¨çÑ=?øL4î–?ÃÈsÕBoÅ?Àъê²Äl?ï6eŸÁüº?¡ªº"VÚ?sPŸ‹fG'?|Ö¨q7u™?"_$ óI÷?¨e¿ks?ìªޘý?£O'˜X?£x;·ýb
?'X¡[ª,?°ó#0ñ4l?eî́?î+6rû?™öžœ&«?EWKûû•?>2Ê/_X?¬÷;³¥Øn?™á°QSaAGN3FGL J1701.4-4654@uD¶°_¯À÷d»k{yÀ8M·Ñ"+À9ò™°?ÎL?ñˎ6.í@Žà®.@àyQû¿ßwB(æË¿ê¾þ¬Ý‡õ¿æ¢	sWvÆ¿ì¯2ՀiUNASNone?•ñKÞÚÿ0?™Ã#çÌéŽ?Ä~Rû?Ÿ›—±É"?êOýB`x?Ãñۑ®
6?ÆuJ˜2Cþ?ÊɜtH?ÏÎÖE?Á°¥]áÌR?âgjÿ¹o?ÌI´æu?½¨!?¥iãáuØ?ÓQ8ª~¢?´þâ´ð¬?â¢`	]L?µ ©8'Ù?´,ßÍ~¥,?¯Èº(×8?½ ¸Ëý³¹?­|¿÷¯×ý?éÖLín£?¹ªûŽ"ºb?vÐ[ÙäÈ?~JÝ£¦)?È
ÈCXÍÕ?Èýüðü?éÏ­7ŽÀ*?ÉN
|Ÿ}?Ö½Ð)<~$?Ò«p´ÑŒ?̜¹¸â£è?À›Ï7úÜï?ÚóÒúR/ç?ÎŽ‰<Õ?ÊT¸¼Ó
6?¬ÀØzï~?ÐüE¦'q‰?°Ú–	ÓN­?àì®ý.?³ºKµ0?¸ïd»y9é?´6Q³)wC?ÅAD8>4ï?¨à´C¥-?ç'ÂZဗ?ºÛ
¶H|OTHER3FGL J1702.0-5414@tçõ£KÜÀ"VÿÁßÀ9°—  À;-X'ßB?í,ýÜÂÂ@𽢍^@ càz(»¿Û}ƣפܿéʓõÉMð¿ë]b¢E¿æÑÑ䎵eUNASNone?æùV°»Ê?É­x.öô¥?žVàq{q?¡0¹ÌØ?Ð'äžXMÒ?ɉtEÕªÊ?æ3(ÄÍØn?Ð4³š~W?³ø=ó¦ap?´ûëï?Í7=óšZÎ?É](èÞ?èHQÜ|ÔM?±EÎ.ÎSó?·È™`÷'&?£æìl'?ÂúkÝYóø?¨ÎkqY?݆Wm$E°?¹)†ã¾¾³?Ã
bÐ@?µÎýŸ?°K?Øò÷*»·É?¶Ïçm
Ô½?ê{ÞáÞh?Ãà\noq?`ÁSvc?"uÜ噃f?ÄxbxW?Ó]¨ÛM?ëüžÄü?ȪÆg?£0Ä׫!?ª"O'g=?¶‡žb5'?»Ù®\Ÿ=H?ìðyqQž? øI0Ù8V?¥æ_¶m¯?"qSáEÙ?«eíqg?–Øé1šŒ?æN>DÂc?­hÐàîòÛ?¾T"èžu³?¤_ðŽD'0?ǜôLÃ}?¥ T`ç AGN3FGL J1702.1-2524@vWñ6;%@#÷Úè'®À:>4ð¢"ëÀ;_$Ÿòy/À
tq£~@	ºˆ\Zsê?ü&C@qŠ1¿ï§Í:Ÿ§ê?äiáp¦cà¿æaW1rÇ?ÈÕ%‹Õ·UNASNone?ïnÚ¼ƒ?®mŠÿA?[ï
àê?\+½‹à?ŒÏ{<‡?®ere'y?î¯ùÁ¼<K?´‡6™c!?sˆ›ü§ˆ?ð"rí;?¢Pf0ã?³ÿ
"A?íOYžF?‹M
•c?˜x$£î?‡wÖa‡?¶?ªÓ¹"­?˜TÂ]?ï²im"?Šû>"?Tã§Ç¿#?+n>1Z¦à?ƒdÅ¬êQ?‰ý›"
À?ìeÛujf?Ò¸c$MÎP?CHr1$›r?KŸÂà«m?¼ª"o'ê?Ò»s‰±õ?ï°d–yöÞ?;48µ¶Ø?]øD~ÅçÛ?e
n€?€'ÑÆRÕ{?Š•É4Ð?îôf¥¹I?‹+]™ÇH?Š—¼æ™µ?|Iî
t¿¾?"'´ŽX
?…Ëòäù?ïîø©œÎ?_JœY[Ë>¶Êð'KÃ2>É%õ ?a}Qf??_I-,Y}AGN3FGL J1702.1-4623@uLw[0À,Ò@ª;À8™Éõ÷¼À: 2:ð?ÑOš+(¼|@Xî>Œ'°@Cà) ã¿êÀ`*76"¿çèáçwY¿éG»¼•XS¿éÀNº«À–UNASNone?½_ Þ:~?·")½
ž?Àñöpéj?À^4eؼ?èžG±Íö?Æ#¿'ŒaÎ?àì¨
ø?ӃH©É?³	8íkÛ?°íÀ<!— ?ÛÞá¼ù?ÑÜÄDVá?О~küä?°Þ¡óޞ+?Ïz
S5î5?³ ïfÒ2m?à-ks¡?·ZŠ/¶ã?ÑŠ+^õÑ?Å3ò7ŒÖŠ?"Ô
ñ ºÍ?ˆEøoI?æɚ{õá?ŀòiû'~?³©üÉf?±æååøm?Â%näåz?ÙÛ0ÆO
?é¯P<•?ÆŽÍŸ?è<Ú±m"?Ν=w²‡?¦Úldëï?¨O¢2?ÉUú8üÜñ?ʚ‰V]–?ҎA*hV?±ÎÝÄÒéƒ?Îë"㯽G?²ZšyØ"?Ýü-"êØH?µÉëÑH'?Õ*šÓ€p(?Ã÷Ø~±¶Ç?—¿¤YáÔ¹?Q%ge»V?䬵sG}÷?Ãßb›ÖŠ¼MIXED3FGL J1703.6-2850@v.¿œb¡¶@™?¯BxKÀ9Úæùž¼ïÀ;1ç£è§õ?ÔîÒ¦U"²@
T£ºM@ЕÀœï¿è¬RV9¬¿ß‹^žµ§¿Ýhm¼	õ¼¿è1[âÔËõUNASNone?춵ÿUá?½ ÛAڕã?š+$ƒÞj†?£C"{ïI?³¿†ã' ?º3kù^Œd?殒ÍüD?Ì5¾1""?»…_ƒ{Ӕ?º˜ý<:¨?ǃäc©?Åžî~^'?êî¥T[|?©²ë ²?¦$#Ö÷	?"ÅKYw?½xÃu¶œ?¤Î¬_"Ç?Þ£KäÚàŒ?¼ÅdM²em?ÁOòx­ç?±â¤ÙÌa-?ص2¡èȁ?¼›óLNžZ?ï#"ÒLO?¤°íåt"#?~ï§T,¦÷?ŽŠ5g	?"Ñ"sjüe?¡
Þc÷A?ìÖ~Ê5mË?À§{;	Á?¢yÚzˆ¨?ª8<÷Ï?°BÁó4S?¶-ý`µÄÀ?îKdîIÒ»?•‹‰÷À4q?'¤™k»(Ï?ƒÿí
(|?¢wdb£õ?'¯*Ë;ÅV?æÁj"Þ?±š©¥Z‹õ?¼CBèæf"?¡xMyÈ}d?ÉcX…äAD?­Ñ¼Ø…_AGN3FGL J1703.9-4843@u1³:}ªÀ¾ «†+À8ÀUM9n·À:¦ƒɕá?ôƒŒçÚoM@
ÉfÅ=@àVŸsù!¿æð¼ÍóŠÉ¿á€Knµ·ª¿ëMkÙ xd¿ïðÊã
]UNASNone?'?uݎþ@?ƒˆ‡6ŒL?겟P…?ÄùÎF¹;º?ÄŠch&§?ĉ¤Íí?"e‰r'?™õ4
èdÈ?ãaÿgºàw?ÃCXÿ9u[?ØRîç¼?ÔÜŠ*?Áú
o ÁŽ?¦ãýfPJ?Þ¨¶h?¶ÁŽ`m~?ØíQ(ÞèÑ?·/o	ß8?®¼°‡ã2?œÊRŒ
?äWü×47s?ºùT™y'"?Ó}­µ?¹ýæÜW?'·r
Yƒ?"pÁ%}&Â?ê¬N§zOI?Ãq5s¨P?Â÷×"ÍEª?'†"E?§
<ó^.?¬ å"§å¥?ãˆÐôyº?½pŽY/ØF?Ö|o,º?¿âòàÕÝ?ÖóÒÏßë?±Ðf˜zµ?Öÿ[¾h"?°Û×Sy?Ò
"o·'?°ZHùÀŒ'?¾ÅuòC?¥v^Š‡ªo?âÍPä&¹0?²~4¬žÉ?Ò´#	?¯Ïg!piÕPSR3FGL J1704.1+1234@@;‡½Ï@=l§qÉpøÀ9d¼¯HWˆÀ;|ƒ-±¿ç¬LT'£@Í,݃©B@ªŠÿwïÑ¿çÌBºÔk–¿è᫦·d[¿ã5àçX`·¿âùs–G!UNASNone?-ïJ±?ƒÒ,ܤªž?Kò¡ês?M ¤ksœ?~W6Y@«œ?ƒz¶ðæ‰A?ïX€¨9£?"ü÷ï¼~?za'ë]ø?l[æFÆ?'ùKñq"&?Ž¼bŒá&*?îQïP–'?""Þ"2¿?'鄼³g0?€³ÄuâƎ?¡ùž®T²L?Ž°83Ñ}\?î:ºá	g)?—Ÿ€÷¯?kê4?däB"Ñôy?ª£CP1§µ?–‰5̪8?ïïÓ'kA?aTKò÷ͺ?;ã#£|?<1vº…n2?Y'÷߁!¬?`dUé'Œ?ïÔi~Q?s—á-'e?b íëgVû?^ÄÏÏtì?hõ"ý繛?o.Wër)?ïfûå>2Á?z|^yuËS?œ+!•t?py++O(¥?†r÷$m?pÅßl'r"?ï ¶·ó²ü?rÍlèˆ*Œ?K×OE:Ç?<'@Eìɽ?†ÝŽÔ?ra㚥¥oAGN3FGL J1704.4-0528@-Óp&É@4̽±¦×À9Q!Ð4`ZÀ;1°(QWá¿ðG˜7™ÊA@
ÖHtÄù@zZ Šy–¿·pCR…Ëì¿êW1zKuŸ¿ËdöU¼¿åù…µê¶UNASNone?ïp•µ!ï?–¿[ô=A9?`¾ÿt1Ý ?`£%
Zß»?ªÒäÚXÓ?–"¸!ßó?ïoÍ^÷?—ƒ_™¹<1?yå/EóK?||ðÌv?‡Eâ$‡O¾?"óS¢©­?ìdÚDÚzŠ?¤®›}W@?¢…µÈmO?'ß9™J?³–Ÿ|þ‡? -@µ9Χ?ëË3¸WK?­X
ÌðZ²?aLZ»?b}Äõ?ÀŽÅ]þÊ?­5Aé9K?ïÅçSÇäl?‡Ð뎅ž£?Xþ1̾N?\‹|~w&?w
։kN…?…û‹ã3Ò§?ïÎCvï—õ?{Ý?crÔ#	C?]±Kµµ¬é?nIûWÁáK?v5B%ð!·?îΟ¦Eq?‰hA–?¬:Àw'J?"!7$‡ÞV?•ÑN/Ɣ?"¶RxM±?î´zÈ˜?"v©RêÌ?Oõ¬ƒõ'?Epýç?Þ?¤8|Ï,¥/?ä®{qAGN3FGL J1705.5+0948@=ÃRü&V¬@;ó~€8Ÿ"À9¤œ«fKÀ;v¬Ö(–?⠝^då@žæ$a´@sï< ¿äËߏG0@¿ëº'fZ¹¿éØ/_Ìî¿ïþ±Ü[‹UNASNone?ïtBy™–a?ˆZ¿võk,?|)•?u;®X¢ÁQ?"¨ÓJÅ?ƒ`í]è?è‡Of^r–?Á-.r•Z?Äïøo±à?¹†•<£?±å"í›?µQ¥p?ì˜X›™ñP?¡etRQq?«h&¿?",'ÿt ?«[,^Dé?–7
ttÖ?Þîÿ¨¨fw?²â`ýñ²à?ÕWYˆ‡x…?´ís»ðxÒ?ÇsM B?­"}в¬Ý?ï»À† µ?wµŽºfòi?p,软?g=¸Úh÷ÿ?qòÔ¼æëÔ?p¸ðْÊ?íT€×/Ž?±êo{â?¬‹ìƒ‡š¥?ªQæîà=°?œX£nï?¢"Úø?î\2+²q"?n0úÆF?žOý24"?…ï4¨>¨%?–)½`µ?M@•fm?éEëBiî?¡…½Á,ŠÁ?Âþ¦'‹N?žðÝݝ'ä?±Â¨¡=_®?–CÏ_9¦‰AGN3FGL J1705.5-4128c@uÕϪ͟¿Ñük`v7jÀ8A[ñ˜^0À9?m?ﲕ:õ@{õ¬"óí@#9ßÊ«_¿çrèf›‰¿êãýVb¿àÙ¯Ü|S¿çÖ·p³áUNASNone)?ŠQí–Bs?š6ùbî;ü?£ÜîH,?µfe^?îeÊz•¥ø?¸a^7ðg?Ä2ÓÿhwÛ?ÊåzGÀ-?¾F©Ý‰ˆ?»Sùou·E?ç*uÄt°ù?ÍTߢ´Â·?Ã	[Âã-Ñ?«+¶q~ô?ÅÑp¢³?­|jw 3?åû´³È¼>?²¶fÚëè?°½ ‹<"í?¼gçÁ€úx?Ž¨Mò#X?šØÅ?rƒ?ímººjce?¿¡Bï?xT»|Ýv?ˆ
՛þMÎ?±ÙÏÏ'Y?Â[z­£Å?í"/Â?¨©;k2?̙<ŋÃv?ÐËGf›ë?À—*PÐ?¹^¼î›D8?䵊îRzï?Оâ??ÊNs
c±*?¯#3Õ¨:2?ÅÁnüX'?­,5H°?ãü~_½'?³z4¬ €•?¨}XG4?¼kigoe? s+"9? HPÓay?ípøøÇ?À—C€)ÓZOTHER3FGL J1707.8+5626@U-þ®û+@B@­ÿ'+¿À:THùn‡À<«ƒ¦é
?ÐA(J29t@
±[UçH@
¨_°Ù¿íÞ¸1+¾l¿Ô}À³l‡¿åY
^¨Ä¿êJØ3ÙµUNASNone?ï¶{Ñ ?tqNÉR?›:Ú=ðóÀ?œhwœ'Ê?ZåeMDŸ?`'l‹?äÿhjøqk?ÎXJÔö£?Ðö8ö˜Z?ÊßÛê™]×?´+Ø͖^A?´þYöa2Ú?ë™3Pÿ?§&k'7±?´
õ"ŸÂn?£"ú~QbË?®Xa£°Š&?—†V/KB?ái²…<¯"?Áó·È-×?Øãè=§¼ƒ?Á6ę™ç?±"Êá¡Vc?¤hdŒT^<?ïÜ
¹§?<†ÝÄÁ?ŠoàáÍR?Žd­Ô
ú?PÈå,W0o?RŠ²½ü2?í\q¿yÁÒ?¶²#G:£«?­‡>Vµ•å?²ß´â…6?™cKc\š?žÉb×]ý?íh¦ï?š;šŸ‰e?¤øØ^ú'?–#׃[ªü?˜pB--'?‡EõúåÜ5?ìDæ£Qm?¤ôÌȪ…#?¸ÔG"O÷i?¢sZp²ò;?"	"â…?‰.ÅWõ+AGN3FGL J1709.4-0917@(d ]Øù+@1¹‹Å›€$À9ZtŠìW­À;"Øzøß?òŸDFx@L'Ûç@·Ðß´0¿à°2x*è¿ää0ÌÚj¿ï¡a+5…??ÜH¿,âGoUNASNone?ìumv6NW?¼É"LŸÚ•?³zжÔLz?·ÜE9Ù?¡³‡2b™?§~E%8Ù?ï?,<b˖?©·{.ƒýÏ?nð?•ìû>Öÿ?-âê°{?¢'¸""É?é;¾6~c«?¬ï£4¤¬°?»uíΟò?£›áJÖZ?º¬!9>B¹?¢ê%…ï?ê§P"#³?¿óÓé5Û?¢Ž¢ò"Ð?´nä¡Æ?À¿<Dzÿ?º_ÛÕÎõ?îE}¨wWû?³¡Û%Õ¬?£Ú" 5‰?°&ýÉ?6Grèþ?Ÿô"´T_?ïĉöt¢%?Œ"¤ä°¬ ?f6±' c?r.s¢ch—?rŸ¬'m±¤?†LC¢W?ì
G¢g/?¡›ý'9e-?®5| ¥×‰?˜…lþë^Ü?©Ù®è£Q…?•kƒž¿û?îÊ£ú›'? Þ$[PŸ?…7øÃ?"È-aÕ5'?œ.]|-W?™ãXÿAGN3FGL J1709.5-0335@1Uœàuöý@4²‰üm¤HÀ9\åüH»[À;*½é§Ï¿Ùijû@&ë$üŽ±@Âb€}¾È¿ç;£g ¿éT_0o½¿à§mƒÕÑÈ¿ïýåғqsUNASNone?ï´ÚAgð?'â+ìàn?qCuœÎ{?qthÉ¡Uò?t'œ<}˜?w&Jd?îwÑ-Ä0?©O>ûN§?—°QGïx‹?'ß7|?™U‰p—ƒ?¤_ÒKÝf2?ëŽApQ…?©&ã]vÂn?±ª¡ðÿQÇ?a5Ç£?±ãRP? Ü¯ ,D?èÈ˵Âçh?±×Uyl? fŽÝÜr:?—és\Õ)?ÈÃ-q}EÑ?°ë.Œ°R?ïâÓØ7l±?g­$­̑?bŸkxŸo?a'šfn?UxÚ®Î?U¯UóC…n?ït$û••²?'Ç`'
¥?€ÚœÆ??z'hÆ®Ì?'%	*ÊO?Œ¸µÛÇûý?íÑvŸf·?š4"ðSà^?¤)Ý}=%?'€¯_KŽ?XEÉ?ÞŒf —?ímâ˜TäÎ?—ö"Ü?ˆê1•+ÿ@?{aˆéœ?±s¥ý4*?–EL÷e¹AGN3FGL J1709.9+4624@R÷´·@B1C¿rq7À:\ìOIoÀ;ðö'9)í¿ñ>ÜÔ׳0@
öÑÁŸ}@í ,ì¿äì>
ì[ø¿éÊñ"žÞ¿ÜI˜Ol¤Ä¿èA»püUNASNone?ï&=κ?"ÊÎ:£#?`¤N'ÒJ?y2›3{Æ3?"]U?"hâpÑ{?ï€ÑƒÄÊ?'ÉÐ*,e?|«ç@=Í?ƒB^.ìu?ÇÉVxr?‡Læ#B¡?íπÔ%܉?—¢~ùúB?'0?BH?€üˆq"?ªoÓâ,?•V"!©?ï?$9‰þ5?‰éºKôRÖ?]Î`Ý"Íæ?YFÑ^?–>'ÇIS|?ˆÃd[XÈ?ïêI¹¡:½?slæ±p??øµV—?M"×í?a·/€BÿÞ?r7Êw(À?ïØë*Ó4½?oûsÚ¿h?a;ÑhÆ¥?\!ÞÐo•?eÙåiê?gYÿK·Oî?ï
S"Ñ$d?‹Ö܆ƒ[L?ƒÇþûSãú?~'"ˆ*¨k?"яè†~?†äjz*?ïßB‹žaÞ?aEê«#é?;áËMëe?0â|;®º?m\xJmM=?`~<˜xžAGN3FGL J1710.6-4317@u'•éᰊÀãâ;ëiÀ8£bþÒÙVÀ:3T9¿ç+"Ÿ¸I@i›Â"¸Ú@6¤€}há?ïÞIρÝæ¿ê×{»Ñ싿奡mV"¿ç"§4•fUNASNone?®Í"ð?°tÚT¡w?•÷|JiµÅ?»É©³–f?ícjÛÁp?³ö;=Lq?Úg.qqK6?Ó?‹ùuÐ?°`aޟ?¬yè.•#D?àÀ\¦k†ƒ?ÒKbk§eW?ËQehc?±_="†<9?Á øuÎc?©ÇO"SŠŒ?äã~""rN?µ¨…]}?ԓ¡Qô¿?ØòÀ&v6?~Ï>åk›¯?J¤*"?åxÖ±ä$h?úrà¥Ð<?³rÒçD?·7Å'tµ ?)†ú4"?—°e9ÊäÜ?íY†{|?¹ôŸÆü œ?æI«Œ$)ð?Ò*,××ö?¦ìunøùT?¦Có"`¢ä?Џ9½?ÐJ¯:."Ö?Ô5Å£}?´>á§7W~?ÀÍÞ1ç?¨åPX0cb?áÆ|d´?µ"•ù<Q?Ü՜Á¹•°?ÁãÇ@Rè?p¼r}q(
?g²O)ï?ás¸ºNÎx?ÁãæÍ\BMIXED3FGL J1714.6-3327@v	9-Œ*@Q]À¥wÀ8ãÀÏhˆ€À:u¡¥×•~?èXç³ê@Ú_c<æ:@ۙ wï¦?ïû7»'U¿é¤f"a¿Î'èÉ
S¿íyü‰ÐyUNASNone?Ú!#P½Ü?ÊÛG}±Ë?Éúµ=d?Å+x§.9?Øá'ñÕ?ÌäÅO]"â?Õ~Jú‹]'?Ô.±]Á¸?Àtddó8‹?¸÷©Ìš?á#Áhôê?ÒMÙðªU1?ÓNÚ®ŒÅÌ?³JZCÒć?̎Âvüê?°{µ‰|Ö?ÞiÄþ{?·@ŽÕ_1?Ó=s/«?Â/ja»?¯˜Â¹`yá?¬yӎYŠæ?ägòRBm
?Ã÷H
þ'?ßÌ߀c?̛á ۆ"?É
1¸š÷Ï?Ä‹Ý:Ѓ?Ó®¤(Á?Êys`—;é?à!ˆT¼Š?ÕæF_N³Ü?Áܧ¢é?»§Ë©"Á÷?ÖÛiáùk?ўœa¹È'?ÞßõX²Ê?´¯¤r
•w?É·W"<ý?«b ®Éø?ÔD_$¤v?³Õ•Gã4?ÛV—Ü€?¿ÇMÝ.Þ?ºÿ•ÄD?§ú÷™´Y?Þ&f£špÑ?Àfƒ'+þMIXED3FGL J1715.4-4028@u¯vݬîá¿òÇAÝðáÀ8çw ÈÍdÀ:qΣf¡ö?Ô©{¨±©@^9ókÇú@ÕYŸ®†'¿ïٙ{‰Ã?äæBÙ泿¯ƒû¿û¿á°ŽJ'ÛUNASNone?ë-¡ð™õN?½¿Ç֘Óv?‡Bø.'¹?"ºŠbÁš?ÁÕH³ðT^?½Ã$`=?Û¢7¢Ù‰I?Ôö®êÛøÜ?°"þ//?°àÜÑs?àDiÅ?ÓªÕ²Š½o?ßþKWõ½å?»½¿`ñ?¹—¢<Ž"?§`5U+¾?ٝŽ¿(§ó?ºmé<š?é‹ÝÑ_Œ?ÂÎÕ°Ì9?ŠeâëA?ˆV_›­µ?È-k™½<?°@éÃíD?í7Ž0?·ß u6%?€l‡z£®G?ƒ…$|j"?µêU¼Dö?¶ê4	ô×?åI¦ßt¼?Ô~1–ƒç?¨ô(…€(?©»
Wž?ÒN-1]è`?Ò"5nÁÙ?ç]Ѧj&S?µ÷ððv'Ø?¯RËþ~¸?ŸŽŠ9,Ûü?Ê´feS†?²ÚÿÞ´E?ëâƒXö¢o?²":zÜ?¥¸E]*ž?}@靮5?½7.2 ï­?±×z׊áˆMIXED3FGL J1717.6-4404@u"^Ñ·ÀÌ2ùQÀ8nzj)i†À:n½º
Ri?ájÜÄÞä@›N•dUÀ@s¿ÀIÝ¿å \ÂVYÜ¿èl¬yxÅl¿ëºˆ×çC¿ãšá?S0UNASNone?âEOk‰L+?ËeŁª?· À'U?·¤S²FÉ?Ս1Ž"?˅à:yç?ÜgZd´?ԉݱBû?¹áN¨ÉQ1?¶¤ýÍð
?Ý QðžÊA?Ñ×Ið[i«?×ÞøeyMì?º
d4»| ?ʑ鹎ùÐ?µ¬ðæ¡?Úؽ¿5,?»æÀ,ÅÇ?Ô Óa]àR?»"´ýo¤?°r	s }?¥cS¡¶?ãáU!}?»»uG»çˆ?ê*aL˜c?îßÉK/v?¥K9×jŸ+?§ø'æ[›?¬XŸ9¨?Áºü6ƒ?æN‰Ð	)?ÑTçXû?°'áfßH€?±™»ê†®÷?Î~)%¾*ž?Í5å^̝?åsôª‰?¶
vˆ?¾Œ°/»¸?¨¼H­.Q?ÌwØw­Ù?²át%œº?ßîoøim?¸[D‡•?ª2[ÁΕE?"É¢bûT?ÜËD¯"Š?·Ì¤Oñ~MIXED3FGL J1719.2-2433?ß&•á(N~@E#ŸAyGÀ9Øïþ¯À:ëьO.;¿ê{—Ùƒ@
ti?´¡@QÓøÿ¿é®z'/Î,¿ëlîïr¥J¿Ó‰Û
àÆÝ¿éu;ss•#UNASNone	?áí%`pX?Ï¿µ'`©Ó?Ž™Ní?B?'"ÈR'?Û0êÈO(v?ÏЫ$l­?ì—û7š?ÂXw'€4?"EˆOŽ@r?˜ŸH`?ºYÞ'O?ÀžC핚1?äÞtr¡;?¶6"Æ*T?´$ÈHæ¢?Ÿ^›=tý?ÒÍdÂ?´r&À·Y?èï5=µ©?¼ƒd"?u"±hlÂ?t`W5ø[°?Ï¥ ½4?¼>íŒÇ	?ç=IS¨k?Ìo:«!¬M?	`ÆÓ/[?€Ÿ9/èK<?Ðý"RîÂô?Ìi@¶SŽ?ïKÙû½?§¨Ä£Á?{ ç×lDk?‡>þÃi÷•?˜NJË1?‰?£Lã®FÂ
?êÖ}†
?©žWó ºå?¦–¶K'5Þ?"¬)Cä?¾¨î"€?¥ïp¾=™½?ìÇ`(ó?¥•ü—^?jÖåXú
?`ŽðPéD?¸îG'ÅýÁ?¥=L€ÍuAGN3FGL J1720.3-0428@1þ}ÔA5@1ìaAcwŸÀ9àÎÏÜKÆÀ;1s?'½À6·$ÄÛ@á=1¹¶p@°§ÀMãc¿åq3†6²¼¿ëØq›Dœ¿ÝèL@[ ÷¿Ï0Ÿ\H¢©UNASNone?ïÇGJJ¸?/¤S¢?2šG'hý?O¢tîRãÌ?{2¶^"ì|?åÜd?ï—{Á¹À£?"ò}†I¢å?jüXcñ3?vÍä}hv?ƒaùx?"gôí?íÊ$½_ؔ?¡_#ø"á/?'ûüO'x?Ä¼ß¤'Ù?ª`3«Úã?œÊ¤–‡G[?ï"Á&ë&?ˆ‡! MbÀ>ÊݲjŒZ>ÙT±HÁâÚ?‹l»3*?ˆ†O/«"à?ï"┤??¶$ 
ô©?SA.""F?ŒâcŒí8Ó?ˆ¥2©ö^?´³'þ,½º?ïà-"ã§Z?r]·ŸgZ?UO+i–û?S
m¾Ò?e*Ո‰")?p%ºnbHž?ïÆÊTLˆ?r֌û7?ƒ:ˆç'?ƒKN4yÚç?'g‰z]VW?ˆÃm¹¨?ïæà¢þ®W?`dBp¥
>°1Nº¿çâ>±±Ç1b6ð?iWX?"?`c­"'i³AGN3FGL J1720.7+0711@<ÿAJM+,@7i㸡œÀ96BhZ\mÀ;MbXº¬9?Þ9ëÜåý(@IŽ"«@Ï€oÑõ¿ãý>QŽ,¿ãgnöÐ"å¿æV	–¤=¿çãr3WŠUNASNone?îÍy<×Í?ž›ù4"¶?•¶§¹Vž?šfØVb?¦2c}É?ˆ®~÷Û?ìcº?›Ü?¿l£¹¥u?±+-¾õ¶µ?²íþ§ý?§n'
ÔÑ?´"ÝUÝ·i?í)³á! ? Ý'Œœ÷k?¤è4eÅÿ?"Ü€ÍZ?ªõ0X¸Rí?•ÏU)µ?âïÖÐíÔë?°b}"'ƒ1?ÆU%ô(?­'äÄeJ2?Î/O¨"¸+?«E©Ðšøï?ï°"‹ßák?£ž²á½?vÈñE‡¤?ŸÖš±»?q%Èá5²?•b-ïöA?î·$ç7~"?­Ä¹¹ß8?—cšZéîa?¡¹h%Š&€?'·Èº¶£)?¢"½"u˜?îè?WQ?‹Ç\-Où?'†u÷ê7
?'ŒJDR…€?'q¦,òHÕ?}îaeTQi?êÊûù'"Ì?™»ñ-5_Œ?²ÕÓS‰ð?'=ÙKs6?¶ÒL〉?"[‡Ÿ¢ñRAGN3FGL J1721.4-5253@u·AJM+À"4!ž¶9
À9Dð(§üÀ;@Ø7d¿ÎÓ鿪X@
&<(zGš@­¿cØ¿ëÈÌ@ϗǿÞdÖB[3¿éó]†T(²¿éêF~OÍYUNASNone?ã®#®¨@ô?È"\M€2ã?ҟ@KŽbž?ÇÉaÔ¼°?¸á\"mì?´láÓw¿]?è[®îP¼A?Í*˜>?²%
|_ëÜ?¶Ë¡¸ÿ?Å~¿ûŒ?Ų;ÚEŽ?æÃ
ë…8}?³5i[rÉ?Ál,£÷ì?¨r˜2¬]?ÃØh#!d¡?¨]20	û/?áw#L'±î?º7jv&´?ºjD¨Œ·Å?¯»å¶ã?Öw(<×n3?¹ø˜zEG?éO¿»—EV?ÂCuÇ=§ç?Ã%®‰Úx¡?À&PèŒ<?®mJ²,?©8Ⱥ©Ë?ìÜö,0y^?Á>ö¨ñÙÕ?Ÿ Æ"Ÿ?¨yÄÌÿ÷?±0Mn«€ã?·{­ˆ["?ìí&¨E?¤-2©z¬&?°('úŠŽþ?šÏ¬LºóÐ?­à'­Ïù«?—2MJ¯¨Y?éM;è¨9?ª2Œ'Ó?Ÿ:‹æ)t€?Sþf!;?Æ䝒¼IŒ?¨Î1`Q!ÑAGN3FGL J1721.8-3919@uÉÑc4'¿¿øs
=³À8·5@L À:B·
èa¿þŸ>+´¹±@A
•iß@Xwœ'"¿í±6i|#¿ÒSüÖC²Ì¿áã6+h¿íbZidz¢UNASNone?ŽÝ~bëäh?•72ÄL?áÐNj­Y%?ÐcØ'Ú÷?Ûhw7ÄèR?ÐtU‰Á­?ä/YT/,=?Õ÷ëY)çÛ?¦a12Òæ?®ý{ð€?ÔÕ'1л"?Ôh0T=M?È/œM±—E?­5B¿Þ á?Õ\ƒÐæþ?³J(Íԉ°?ދ®ÿl¡?´à¯ËOÃ9?á–Ã)Ï¡?ÌA$bŠå?yÑ´°¦Ço?…ù%€'?Ük2ÙF,à?ÌAµ_¦a\?z°Ëa­?Œe—vŽ-©?ÛZFÅ-¾w?ѹÒü‰p?⶚9a?ÑÁMª‹b?é1Üøس$?Òyž"֝?X@¾#Ñ?¤Eý'ðë¬?Ǎ"#Iu?ЙW@ýt?Ð¥¶»ñç?¯4p‰¥½?ÔXX»F×D?±.Òd1?ۏý6Ö?²4™W?äWˆòy?ÅM|¤Z+´?S@VOÖý?`Œ­VžŸù?×=¯™ÇM?ÅNETÀCMIXED3FGL J1722.7-0415@2~µ^ñýß@1"BÇû¬´À9‡YûôÙÀ:æ+Íä$?ôëG©·ÉÛ@7´»³õ»@[ü€¿?ïûǪ+À¬¿àñ†»»¿ènÂ+øÆ¿ïÿ›ÞIàUNASNone?©±÷(:ú?®^s‰×³?ëÊΔfî?ÀÅhÆN>¹?´ÐÌ꓂?º\å3K?œ$ÃQû€?®€;
i?ë—Äb£–Ñ?À7ÇwMij?¼@Ó¼¢"?½dGà
ä'?É28èºû$?¯݊[Ïd?âVrØmH?·‰Õ^O'?Íu™KãO½?±Èm3ãq?›E/Â?'… ˜…U<?éÒfâ(r?ºAë×Ï?ÅM²tu·?·ÁÏ×õô?´d¶oà…?´Æ,V—ˆÀ?èËg/l²¹?Æܨs7kb? 
\ò—?Âņàž*?¬2¥V­?³,øgá?êíÝ©œy¦?¾
ln×èÎ?º‹˜¬ø?¹DSصÀ?×¼x³½Sª?±/'.Ûð?ܱ55/Ñ?±ƒ«@—-?Ç$ä.ù?©<@­W,0?³`8TË?ôA¦€—F?ç'œ›	d?µÂCXè8?ÈGêòŸÉ?±Â…ŠPÍäPSR3FGL J1723.6-3646@uîΤ¨ÁU¿Øsš×\HÀ8›EÏíé}À9¢P¢¯ÂÑ?æ%c¤·@
Áñ§w¨®@Ìh€Z?žŒä¹ÚU¿è,E·3!¿ä*ï-†P¿Û£±[¾RóUNASNone?v–ìÑß
.?}ªo³¡Â…?¨–=S#'Ë?´À‰D"Hô?îInQ
?µw'y¢ '?¼oês¦ÀÊ?Ä/Û@i7ã?´ózNýH~?±æ׍ΒÓ?éӓh'0Æ?ƜòèH?í80‰œ?¨`ÅæŽ1?Á$óCGí?­äÒw¥ ?æËu)!âS?³{úÔïq?À·«-üή?À؝°ª'J?‡SŠî:m«?	4t5bâ?ëtǬe¾?Áz¹~óÑ?mö0ˆúN?uÿÚe¨?©k`@™p?¶ászó|"?îKSÏF4ÿ?·i;¶mŽ?Ë-«>²˜C?Ðraê?¸>†Ä?°l²©âœ?æ43™G‡?Ð=ƒYÍb?ÉR·ZÓ=Þ?¬'ôºÍQõ?À@èTÐ?ªU˜l/?å›L/¿œt?²zpnq¢?ÁÏ·@|$œ?ÂtÚTl5U?–¾ŽånV?'cA‹»?êۜ;	–W?ÃLq'êRðOTHER3FGL J1725.0-0513@1ìh¹ý½0@0&cAøÀ9´â:¸cÀ;ÙÁfg¿ô¸Î¾¡@Û\ÁL$@%ÄÀcÝ˿ǃõ…0"¿é1̋‰`'¿àz»÷¬8¿Îxí|›UNASNone?ïr—š™|q?'ßgNÛ¿¶?]–rÓö!†?^¨"?§K1ã?'20©Á?ïuW°?–j¡:Ã~?pî—M;("?x6×¼AË?ŠA^…v•ì?"?yGú?ì[—M?©[/ÈŁ?›9,DÍ&ž?‹}îëv)?¶Tõssºï?¦ƒ¿†¨?ít
º9š?¥FžÙv2Ê?3™ìò	?7âe0RUZ?´KøB¾W?¥@kŠO•8?ïÕ/<·?u¾öÿ¢?Pâъc~?Q‡{=DÐ[?q`èó}÷a?sú‰ö?ïתʪ™Ø?sUÚBý8Ï?Yžüp?T³I­ð×?k…·:šÐ?p« €¯7?îÕo)L?Ê¹Î͕æ?ˆù1"Åy]?|€?â?˜Õ'>c[þ?‹Ùž¨_Ø?ïJŠÇçN?"6u­c? ŠˆR…«±?Z©Àn¿d?–'õ÷˜œ?"-稝þæAGN3FGL J1725.7-3555c@uý—ÿCB¿ÏBwß4®]À8+Þº5"À9O·Xâ?Ýd"¼Ð@dZ­ Œ¨@Àè€1"¡¿ì·ºýþ";¿ãP¨¸V¯J¿ß‰DL`*ã¿ëw­þwâUNASNone0?'E3Lîu?–òŠ½þ?ÜÎÚ;¨Ö+?Õwyæ˜GV?áiG†G?ÕLYÙÔáÞ?ÂA†¨¥ë?É
"TؖÒ?»D‰©®Üï?¶âÑ"ïa?è
*_úç?ËbboO²ß?Ã4uP?¨Ðàá4ku?Óe$'¸ç?²â½Ll¹>?፠š)ax?´LKýT`?¾q¹`´?ÂÍMV±"Þ?‰ÈÔö ?‰àÍÊHš?ëÖNŸ?ïh Xm³?'tËÓ|?‹ÏEX&?Þ$(@è?×Þ¡ÓqN?à¤&¿¡.þ?׹ه'¨[?Í ¾yÖcW?Ј›L»ß?¾ðglÜÞN?³ò‰2¹Ó°?äÙÃtx;À?мø÷֙?È}Ô|?Ÿ?¬Ðl ‡‡?Ҝ|'mØ ?±HCóÚ3¼?à'LËà"©?²¸ÿYt·ù?·Ç}ò8?ÂJ®úÔÈ?•"¶Dšð¤?ˆé:º½µë?ìZjjìˆ?ÂƯ˜DÁOTHER3FGL J1726.6-3530c@vÑ·Xâ¿Æ'ÍúI\ÀÀ7£-0º²ïÀ9‹Àނ÷?òÄïc$½z@eÛ­m0@u¹_݋6?ìဌò/¿æÐZ\± ¿æRT­p)ø¿ê΍Ÿ:mdUNASNone$?p;KSÅ?qû`:ª¯?Ϛ³R¨D?ʶRo?çù|ºÕm?ÊՁ5c}î?'"«‰Fç?£þ®¦ƒþK?Æt­Ö+_?¿U›èÔ?]?éÎ7-ò4C?ÁCån?Š?±U4
Cwˆ?ŸMe§tb?Ô<õÑuJ|?·—sØ"¿?ã¶Þ•eò?·"ÃÌ?£†¤[c?¢V)£Ú"ž?·¼øÞˆ?«ìѕˆ?ëãÞ@É/?³…5‰y»Ù?[zÊÛ2ќ?eIÀ§`Ñ?ÒH"÷Ñç?Î*º&4¥­?æèP3Z\?Î6Ú|ã«a?Ÿ(–5ܼÌ?­åª"aÓ!?ÏaµÎ?ÁÉè‹?ç.N	M[¨?Ãú²Z¨Ÿ?¶>:''?¢kÁœ§qó?ÔFª¬Þ?µ]"/í½å?ãã{SÍ ?µ÷P‰'V?¥¥}Qµ5t?©k'ã0«2?¸Ó3xP?¥ù7E‹?듭ĞÕï?³mA¼OTHER3FGL J1727.4+0634@=6cÇOµ@5¥yžQ?À9‰/Þê܂À;:³In?ï.ú81¤@W]"Dù@&À36c¿èEw¿çx¡È£X›¿êÝ\îSÁY¿ïùAû«UNASNone?í6ÊãKi?­ÇÅ÷½ß?±Ûʤ¾
É?ªÔ‰-‰¼?'·y¿/Ó?Œ_¡¯Ø™?á{ã¼Ç?Ç¥Y´"à?×<Þ¨A}#?ÄK¼þë?ºˆ¦AÈ¢F?¼nA;´Œ?è‡6"î´ ?°[T}°°?ÁeêµÀìš?¦…'™?¸úvnÀSÍ?¢‹ÒÓfN?ͬö˜£$ˆ?±¯LDË?áÐ¥9_ó?» g9Ü*õ?ËtÝe?°•¸‹è¥?íòèê²q?¨96Îa?«_âkTÐ?¥áª
0õS?…Æ;¢¾<ƒ?€wükkøè?é:BÖDm?Ào"ëšöÄ?ÃÕÀÚXÚ?¸s·˜?­Ï7T7â?²"9ilÑ?ì4ƒ¹Í/?£')*Dž?²ÙUÙ;Ë&?›×ãjÞñ?§®ý¢æ?'÷œþ)Æ`?Þ㶼GÌü?­¢^Yꑋ?Ø̒EÎ|‹?°7ö`Ô]?ÀŸmûÓlñ?Ÿm¿ì¬ ŽMIXED3FGL J1727.6-0654@0Á‰&"Ï@.AðÃLÀ9A 6×,¢À;>Ä`î?âÎqê iº@H³SÜK@¬M@O¦[¿âC<}‰ÃŽ¿èó|Š¿äw‹pû¯}¿ïÿ݃±Ù_UNASNone?íâ¶p6kC?´šÕÛ£?ˆ®Lþ?;?ˆú⨹ï'?«©¿©ð÷?³|RH¹@?éõ2>
#?ÁÜ eµ?¿J(ÜÜÔ?±[dnÍ:?¸¦-'2ÂË?ºxܨÀ†¡?å¾o›æ?µpŒØɍÜ?¹ÆÎ_#7?¢§JÕbÞÍ?Ì"܎`ÖZ?³oTÕýõz?ے`C¦b?³'r©'Õ?ÉU­2ÊúÝ?¯¥åb‡îþ?×ÃVÜ0?²rxN'£?îçÙÍ*.—?«ñ'c…Ü?yrWŒH?|ÃYb7R?œ¨EÿŸ¥%?ª–œFï"ü?í3äàâ%?´Fçõfq?©•(â"?¡¸nkÏy(?£Í‹£x?«¨Œ…ò¹??éñ⻡E?°8]T†úb?±§
Þd֘?›_ÉuF¬v?¾ÉßB×QF?ªÄYˆ¦e?å–#寿?©¦ÑÉ?Â2@[²$Í?¡ˆp €Qj?Éwg·6?£́dAGN3FGL J1728.0-6446@tvÌcñA À0MÛU%ÌÀ:¾[
À;¤®ç¸5?™"¤¹É"þ@YKÞzÊ!@Nº€D¿ê$­´Y¿ç8Q¥¿íÀ¢ox€¿ïýb¼¶UNASNone?ïÉßH¿%^?{ý–ÙJ?hƒ¨ÿĘ?isñçÕæù?mµÙÓ\ê?ss¬­Æ?ì*ÁÃ[?Àb!y2­
?¥Ãû£í?§çH8¨èí?³Çô…?¹HÕ?í¹<eü?ž[Ø,¢+?¨—OŒA?'°"ß?§¸ˆê?'ûˆ›Y5?éÚ¼ql?±HÓ-!ë?º@u;Ä?¬L³`4á?½x´ábtÙ?¨é^^ø6?ïÞµbLü2?sÐ>g?^¦Iöƒ?`ä4"i‡é?a÷VAÊÎ?k.BÎPÄ?îÔ…%ÌÌ?¨7]É»ž?Š5RQ™kE?á}bHÄ?˜bÆ7¡Ü?¡Üç[ 8?î')gÏ¿h?‹ºü1g¢?›cž~éf¢?ƒÂº'ï%Ç?'w4…fÞf?~*«Nž±?îYë÷4d?'uí±¸Ž?–	F¸'¥†?ƒPgNY‡?ž¹:iusü?‹xLˆgï³AGN3FGL J1729.0+6049@Vr¦óõ/Â@@µ‡?úÁÓÀ:WQ§'€¡À;¢µ'ôcë¿ëMT¶T"@ÒU ˜ÑÉ@-ž_§'¿è`
rô5¿á/èSÍÜ¿ìDƒŸÝ+¿áôÉʨŸ
UNASNone?ïÏÝicW$?xç {s³h?q/_ɏ-?u§L'!z?[‡¯¨û—?];	úSe|?ïKôiì$M? ZG~«µ?"°Àç6;™?'çå³ÌÁQ?ˆR$–áy?•"凢®é?ídŠcú.
?œÈðodÎ? È·qúKê?]" \*ž?¨î¢P¡K?•¾=Þtú?íK›ù˜'?£z~ïpÑÿ? Ðl)ùí?Ž¶0LOÄ ?±¯+¿Ö­?¡¤^=©×ö?ïñPôˆB?\¢4žq]y?Pàc¯1C_?Wr7Òj §?HûgnB?E"5v7Â?ï̇Ҕ.m?|ÈB
#âä?g<×±ã(?kæ­õÏV?l;U©pJm?t;Ûñ«p?îÛÏŔc?Nrï.ù?úâ!^M?'Ó`‡ ½‡?"£#ësI?ƒ.K¡ÏØ?ït©ªÍ?|Q9D£Ã?`ªG›°Ú?SÓˊ%´û?ŽØêõÿ6‡?zßëeþ²YAGN3FGL J1731.9+5428@TŒ]á\¦Ê@@"ð^¢LÇÀ9Ò®Q·'¹À;Ù
£ÇðÅ?ÜÑ-<¬·6@
_hT'I›@7#_ÖS¿çފƒu•¿ë€"È×Ë¿ëÄ@Hq-¿ïþó…?¼ÑUNASNone?î†S‡Aù?£f'ûgW?Œ:ìB¼p½?ŒB-MËM? Œ~˜«@?Ÿ—Í©¦?âÉL{Èg&?ÊN™^?Ôg´¿ºÀ†?ÇŒ7?Ð?¸É#­«¶?¸x9;yÂ~?ëFfގ–?¥_qºä_>?°35 0?•þÆ/~çŸ?µ™šM# ? sƒÊN?Ým!ëQ$?¼÷åûÙ
?ÜGÂÑ@?¾Ù:6=ƒ?¹,m~Ñu?­,"}bò¸?ï]€}؍?'‹҈H?~£aJq?|-?‰goE ,¸?‰ 4‹KC?ë:/KrM?ºë[¡D"?»Ü¯vƒG¦?¶¸´6ßØF?¤£¬_Gwß?¥njT¨;?í¾ÞMu?–Ÿ»Ä';ø?£rrbmê\?‹ê"k´p? ¬·å×W?ŠÔMrã(?ê˲á>Hæ?¨
¶7@%b?ÀÁ	¢7šC?¤vî/.R	? @«i@YŽ?•B"™˜áAGN3FGL J1732.4-2709@v×Ûôˆ@8™aeu¦À8º­²URBÀ:Wè+Íä$¿þëÖj…Yò@"v¸@ûԀ Nj?̧¸ÃL賿ê•`;¿Ýû–EɅ<¿ç"´ìA˜bUNASNone?Ú¯®'Öà*?Î0@"÷?¡•õ'èYú?¤(Q'JÄ?áŽÉd–
L?Îáþ9x¾û?ê?Ôƍºá?Ï{$£ùCù?3H©Ryi?œ²^(Ø¥ï?ÄúCÏñ?Í×ɯOÓ?֕¬6v«û?¶ó¯"u¡?·A:`ߘ?¢ê›ìd¢?áÍ™&Eÿ?¸%Ô]·W?åÄÐK~Ñ?ŏÝÀT*?CЖ¾Tø?M…*`£?Õ®"?ŏÝvEà?æ‰O…µr?ÍqsF~?¡üÙ»	æ:?¥ÜÿÖז?ѱR)åÎô?Ì.ϒ52x?í²unÓ.?É+z^r°?†iß)·,©?–8­ÁOÞ=?µ
0m,¿?Æ/¦?àܽ=7Ãç?¹3¹×+ê?²A$$±í? 4ö²Èks?ٟ5<X8?·æ`5?é<ª™'XÆ?¹¤fÚ³?-'b†v"—?28~r
s?ËñAÝVC?¹¢\V¾ËMIXED3FGL J1732.7+5914@Uøo?Rü&@@ƒô#Rë_À:úkáÐÀ<®âô?¨«CLš@)¿A@S f'?ïŽß{r‰'¿å?Ç7%tó¿ä{þi/¢
¿ÅQwnUNASNone?ïäsO-×?gK¾Ôx?SWò@ŠðÆ?U©ÍÛHó/?aà·}É
?ao¼È¹"?ï}ÙÚå'?•Òa6B5?{&qâþô?"cÀ;"WÍ?'öP—Ý­Ì?ó–ÅfÂ{?îH…®'^ž?"GFüÃÔc?–JÂwÝ|à?Š¡—ù"? RC׋»·?ŒLéa§?î'tší½Ä?¢:2Z4Î?"ÕÆFÄ?…n£J4ð?£[œme\? Áñÿñ™3?ïóº²÷l;?Tâ‹»á?B€æ^÷Ì?D§OW[§‹?N•0
eÉ?M_àH_?ïÕ«Ø­Î?u¹úª#?bÅ'Àª¤?bq¹
¾¬?h6;Ÿ'i?pˆdç+	þ?ïs™æס?‰Ý[YOÏ?‹Î}.Ä?ƒ9·hÚÝx?ŒÔœ'Š¼æ?»r6«ô?ïÇçQ…?yÇb7Í?^®ó¯Ïæ?[ÅÖÕätq?të ³ýe¡?v®=±ü9AGN3FGL J1733.5-2811@vsw[0@#lfZ§ìÀ8Ã=dRÀ:.¾ÐŠÇo¿äРÅœ´@b£S&@é¿¡Á¿ÀŠ»î‹Áó¿ëòƒ
¿åàèϦŠ³¿ã—KOx}UNASNone?¢B—±
o2?¨Pfpˆl?Ž8‹˜Â1¨?ž]öƒ¿§?îbôV~'Ö?°®=ô
?â=¡jb8?ÓäR•á?¥2éÉH8?¥ôxeÖïG?Øßg"±l?ҟEE•6?Ы§]Â?±Lt;<÷??¾,3ûB°?¨mbÁܧã?ãä¥ôXj?´€²öjˆ"?Øò&›þ¬L?Æë"â—(?n®Yøúg?fl7¹
Rþ?ãhå¥Q?Æýì ò?£R˜Ç?LÐ?­øU|3WE?‡Üé® Ö?–½3šà°?îkbÌÓØ°?±Œé£Ø§?èèÔ>·Ã?Îw˜¬£{_?"øA^ˆæ?ž‡à.Št;?ȸP'Æo?Ë¡L"5à?ÖÛa"C4ø?³™†F:'í?¼'ô¼ø‰?¦ÅG´?áð¦Nfs?´*Ä»æˆ{?à¯éÏåA?Â
Ë2÷VÂ?i"1ycà?YüÐNÐ0N?Þm%¾'±Õ?ÂöcÝ½MIXED3FGL J1733.5-3941@uØۋ¬q
Àâ1ƒ/ÊÉÀ9&/ŒEÀ:É+üLû?ÞC+9zÜ%@­OoÔÏ%@×àŽ¾¿âr¶ì€Ø¿ê'WMKt¿Ø'å¾òTؿݨ`'CLUNASNone?ì>uGðk?¶Ÿ; ëNJ?v#ÓÊc¯?tµc¹yè?¼ª%Óêp?¶NÀ¬ëÌe?åw ~æ"?ÐÍÇ"ÌM?¤A6ˆÖ'n?£ß&ªYrr?҈˜3¬Äˆ?ÏY×%°?åòɆÏÆ?¹Â|BÄì?®>¾çèÏ:?©îéf½?ÐR•GÝ1?¶÷êÇß?æÇr3½á?¹¥À¦EEý?{îcô9ÙÜ?~rMF",ß?Ґ·‹z¥–?¹{ü"›;Í?îV:éØBÄ?§Xqßý?gÜZžn?iØeµN?©‹ºÁ"?¦¿ý†~ï?ìj};-í?ÄmëJní?"p¥$TW¢?˜#kâH¬d?º 'ÎÉH«?Â~z"U?솩'Ö¤?§²»6sðÃ?›vüãJO ?¬áY}ž?´ìô6RŠW?¤e:‹Nú¥?ë®uN¿3e?¥ÇµrÔc
?ƒÏrÂó±?sŽ¼Á¦È?À	3˜¼W'?¥8	wF4LAGN3FGL J1733.8-6056@t³‰ßrïÀ-‹:%•»¿À9poz^ÙÀ;'2{}NàÀX×æÜBŒ@%€˜Á­_@§©Ÿ¡—¿çN"kô¿æ-ø°R¿ì"ùTs¿¶G€‡UNASNone?ïÖøþÀ '?o4ÏS?coÂúËÁ•?b"ãí™W?e—>-¶¿>?e|éŽ
DB?ï|]g9?Q¼ý?of½ÏÝç?yî`kOE?‰"Nî×aò?‰šû}ìX?î	ÃÁÇqT?•d5¾æ ­?—æêö§"b?"ÍR
%óÔ?£pNf}S?Žêÿ–'?ï®Òðl(?ƒ²ìÝJë?ö—›÷?(€
ÛU?"8;æJJ?ƒ­0hhJG?ïña?UéIyØss?J Œãw?EîMü)(?P,¹7{tV?M\e³½š>?ïÓ(††íE?vÿ»÷ê?WVßV-†e?\¨áöS¨¤?p–ÅQÐM?qìÙô×ô?ïA¼s–Ù)?Ÿ,¤¥p¥?…')}ŒN¬?t-Â܍!û?Š¹­ës?s,-
‹U?ïóºLl•*?SÚ*Ñ`k>½Ë˜€Ñ®z>Ƙ߶æ "?Xƒô¯Ä?SŒöP²SAGN3FGL J1739.9-3124c@vT&Á½¥¿Ð†êÕÌOÏÀ8\+xSδÀ9ò5ýé?õ€@tº<&@zž¬¨ë@P¿ "_ž¿Ü`7˜r¨¿åӃZho¿çd'²ÕŒ¿èߪ4ùyUNASNone<?…ˆß^¶þ?ƒÕ#1Wñ?ÈZaPä]?Äà†
ÜȪ?é"D.ÇØ`?ÅQ"TŸÙ>?™"Êh<¬
?££
Á~?Ç5ÑÚ9;?»á"§ñÌ?éeí6=˜?À%]vlˆ?·	®VIv?¡Õ»ó?È|P†]Û0?±
†¢Ý??犨KIf?³Õ ":#ø?´ðfÂZA»?°7´ {Î?ÀŒJ3ˆv?²gçöÂì.?é>ÏÕQû?»`š
ªÛ?}–1ZoÕ?zаmVÖ¸?Ìe‰Ì¥"?ÇöÇî§Ï#?諍?¡´#?È5濚½º?«Ø#őv?¶&qÑû÷?Ë
üC™&?¼ÞQm¾?ç¾²éÝæ?Ä"›å"?ÃZ4ÎW«&?§ÇJZ<?ȗÖáðÔ?¯YŽ.	?å}Dñ™?³¶!ŠuW?¸Mý7C{9?³!ätv?ÉÑôoå&q?¯»ž"]Ó5?æÃ=p½œ?»½yÑ/æ€OTHER3FGL J1740.8-1933@º¡<ü	Ñ@NkawêÀ9‡¸·lxÀ:ÚwNëö^¿ý133‰o@5M6¿"»@²¾_v³¿àaKw«:ß¿ç<A³¥£¿áv…¥ñ¿޽çIÙEŠUNASNone?înyYLi?¦æÌ2`>?]uSû'ûu?ZÕdˆ"5?¨,¿ÇBÙ ?¦ž¸jÔ¯ü?î÷?«ÖL?·ŽE?F´<?yºT"äªé?'ëu)æ?«™AƒM¿á?¶Kfœs?é97+á=?³9û(0Éí?¦=Å0ÁÖß?•"Zü³—?ŋ²	kÓR?±*r ×Ô?ퟱ¥Ý}?¦ÚJ&ÔP? }Îýå?#˜¸Ë_ì?²ÿF3bzk?¦ÕŽ~'¿ü?ïUöNæ?L¹`<Ä?G«Í†*°é?F‰ØԝN€?‹/Å¡|•f?ˆ ßg?ï‹÷ϧ??–ƒ)uOZ?bCδv?i3n±z?ˆq_â¬?"¨"‰9z?íÈqö^ãÞ?ŸÊŽZÖx8?'´¡	Ó?‡•	›?ªØIŒù¿?›~©¿†²?ï2¿3öÁ?ˆ	Q({?ú»˜oR?Nj4ÒÓ}?™±Ëqê?ˆ°œg¼AGN3FGL J1740.8-6755@tRg ù	lÀ2¼8…	ÀÀ:Fšï/À;»\´5ýÀy
‰ò@`›csAì@O蠒Ý¿ça¶u¿èÇÖñhãn¿á'Ú~U	¿æ)wT—©LUNASNone?ïõiú3|?RœBRú:§?0]
O[v?4©¡O8l?PäÔmyM?PË֞*úŠ?ïuÈŒW?Î)œ›&™?oðwÚ~§€?wl8s û?Š'°°Ñ2|?‰æÒå°?'~t$?UŒŽ4­?‹C"SrC?uˆhi¬ß?Ÿ§ÎÏôY?‰71cˆ??ïôVÿk0?'yü9Yº?ÞQSÌ­é?#§«òzê?‹Ï-—kU´?óÈUl®?ïëBp_Zü? "x¬¸P?aÊpëM§? ÁïzÖô?7˜úùŸÓ?6Kىu4°?ïÓ7PŠm=?r ƒ¿¥å]?VÙ2a€;b?UfŒã¾?p®?F
?mijfv¿?ï{æìÄË?tÈôØÞî­?y8ß±A[?j肹™ñY?"j6l³
‡?kÉB¥Ö7?ïë— 1h?Xeòd;J>íkÔDmó>ö‡j†lp?dÏüä`÷ð?XVnIPUTAGN3FGL J1741.4+0938@@âñ©ûçm@3ãý?[_¢À9vèõø?AÀ;1ÿD]Å?íº^?rÓÿ@À9Iøœ‰@ø8`nª®¿ß؎Éöj¿ë¤g¥£	§¿èpp3 …¿ïñ'½pI¥UNASNone?ìjCND—Æ?µFB­?«÷
œ'Ò"?¦÷c
jÏ?­dÀÿ˜?°äsþ?䝱y4I^?Åÿ¬}³?І}à"?À½Xcvûh?¸ø|µg"S?»QPàî?çJqtÖ?²ts$9ñ?ÂÏZ¾	?¦¼D@+&?ÀVjÖôª?©½<¼÷K?ÒàŽ1þÍ?²õÅ£ê?Ûx×l¸åå?¹Ö¡"?ѦšaHLþ?²°xï…'?íƒúq(iß?¬k§GEþ?§!° c³?¡þïÞÅ~Â? ž¨K^^?¢7#FšÝÖ?êܶ'ª?»×®h?¼UÅ.rÚ?±‰ZÑ÷¥?©"7e|D?°j Ï]°?ëÐDe'N?¥4¯
úAì?³è¦žÅ…?œ­©	èÐÓ?«*lhž?–#S ¡Q?áiÀóûÙ?«Ã£K>?ÓÁH's"?¬=-¼Õü?ÂÖõžìÙv?¡>Ö¶wÏ.MIXED3FGL J1742.4-7237@tgßã*À4à´Ê!!À9ùÖÌ*žÀ;¸ßR,¿ÞÞxžÕÌ@ 3&H@aÌà,¿ìé܉ûŽN¿èú¬Èº2¿â2úûM,¿å»¢ÆBUNASNone?ï{ Ø°¹N?§'¹³·?]"`Þ­A? <–uV%?s}©¨V?£±Dª*À±?îÐáÈ+u?«;§a]†ý?"!šÏº•û?"õ¿gçùW?›Òùœœe?£ö?vˆS"?íiõÛ 
ˆ?ž^
Îc‰?—»4VÆK®?ƒ©Û¶=¡ô?­ƒx¥?™?SÑ.?îHg:ªS"?›÷Œíò?r×yá†ÚÞ?lJߛ]Hm?©xWî?šàš×S°Ï?îv™××í½?Å¥%«"?y5Đó­?™Õr¼Å?¥o©ñ€‹V?Çrâ?ï£Ä;w`?Žƒ"ë¸+?j£f?wëæ]	¢î?€f-Ħé?…Ÿ‰²t?ï#õ–M<|?†aÏ)¨®?…sÖ¬îŒÅ?~Ü^š%æ?Çaå"	?|f—$Ÿ?羽ÝÙÃ?uö†,õïj?XA¾ž4?EñtE4–µ?'Õ F¹"M?tÓ´{|âüAGN3FGL J1743.9-1310@*«ø˜,²@ õµØ",À9†·5ŒÀ;
3­¬v?ñ5£Ãi Ö@ó»Æû}@ærÀ'Ö¿çpïñü¿¬ÍÆU;%¿äv–9½»ã¿í¬ŸâKgUNASNone?µd뇻T?´§´r4'?ìåЎù,§?¶ZM:†¾¿?‹d€
¿|?"'"ìqV?ÚƑ|ó#V?É4â¾YJ'?Ôþm¯—?ÂÁŒzªÉ ?Ð:ï]E'?Å«ó°³³î?ØÂ@Šg?µ-ŒÅ¿ ?Ý'K\Ÿ?µ<Ôõ×Z?Å»sã@pw?ª¥wqœ<œ?Õo÷§×?µºì#bh?Þ0Ìö%Œ?¹¡1H\?Ⱦy¾Ä¼?²çŸâK¼?»Ô+{¯?ºÀ'âã[ý?ìæÄ*øã?»üê¡ÉéÃ?‰å¶OHA×?œ(kä<œ?åû§£?Æ(sZÎ?ȏ	+ç~C?¸yë?³Ý?ÃTªåyõm?¾hu›sË?ã@ø_Åø?²ÒS½
p?ÒûõÚ7CŽ?°ê³SqD¥?ºe"¯O?¢a¸rS®?àå¢ÙU¾›?±•KS=ÿ:?Ö¢;jJ‡Ê?±C´Uû?¾Iûsnü?¢ÆV*Íì¯MIXED3FGL J1744.5-2506@	0"¿íÁ9@¤±«VçÀ8&ÆÌ˲À:)}uv¤¢?Údúr™Çß@
Ó:ÉT;@‡À(N©¿æšø2šö«¿êñísˆ¿ã÷[ Üü<¿îart`UNASNone?µÚùôîÁú?»…Ñ¿ê€?Ȇõ£ÁÌÐ?ÊÆÕÃQµ?ç"ãXÄ+,?Ï«0Ýdìá?Íѹaœ8l?ËGÕ3+?Îü–X"â?ÁpaÖ£?à̎ÂÌí?ʬÎÞ'œ?Ư…dz;	?¯7ŽêA'k?Ï/&€"²L?²⌏‹r?âˆTíd"L?·íãî¨:?¹6¥B?²W†Ðmj?¹ìüuºtä?ªß,ôg·?雋Ðiu¡?»Ÿ;¼f²?¡Íßz݁?¬ßóïF6€?ÉÜé1~ʃ?Íö9¶Éx?èkç¼:§?ÏÁT|6ºÛ?Þ°Áwë…?҉~éêêÅ?È£Îώü?Á.ƀÇ*?ÔýWÀ–3?É5ªW" ?ÑB£a!5¸?°²Àþ¥¼?͆î¸@ë?®š‰bý–½?ßùåCç
'?²«²ñmÏ?ÂAÖÎOÑ?¹'Ǥa!B?·&kýé #? ‰V	ßÃC?èŠí
s»'?¼ÎÎ;¯%MIXED3FGL J1744.7-3043@vfÃóà7¿ès ôlNÀ7þ+i:V=À9Æú¤vln?î&U)s@F¬RÐÝ@æ›_Â]]¿Þúê—c	¿éðŠtÁ%­¿äÞ—fñ¿èÕ¨5
EKUNASNone?ŒË¹§V¿?M(QغÂ?´fÏ2éÈl?¹Ôä¹þi?ìÿ÷2À¶X?»ÁrTõêl?³¢(-	'??ºnJmXëK?ÀäçÇ`7‰?·Zl¯˜Ä?éRËx?Âõw½ôR?¼	B^tT'?¥š ×ZØ?ÏJ1©'­d?¶™Óçxhª?ä¬KIÌÊ?·ö¾–Hï?¾×]…¨\;?¸däAnÆm?¢£#ësI?—Éñèç?êúâx?¤?»+ÁyÝf£?ƒV•xi÷?‡

xÀ?ºLWÕ©Q?À$aDy½Â?ìi¥8on?À®È[_2|?Àæ`ûb?ÅSµ–œ±s?ÃÃzڀ?µÈ-µ•¯œ?æՙåøJˆ?ȼbÍ»ÆP?ÄfíÊÉ<?©‹»G"Çý?Μ*Uòƒs?²­7èy‰?ãQ¯š3?´sŒdˆÝã?Âøjèß±?¼nÖ!Š>]?°n­2?Ò°?–âԚ"_ä?épì?Œ.?¾Bvvm´ROTHER3FGL J1744.8-1557@&™»'ˆÛ@€ô"'òÜÀ9Rìzçý«À:î__áçç?å+Y Çd@ö–²‰›@z‡`%¿©ê7'õƒ¿äõþš'Ö<¿åjc㡜ë¿î–"	u°ÂUNASNone?ÕZ¿i6û?Ɩýª\¬Ì?ÚÛgÆIH?˄Šw×kÑ?Ð
=zM½½?Æëö÷‡?ο~Κµ×?Å3{dq»ü?Ùĺ	%É?Ě¥E§Ýˆ?ÖۆŒáŒ?È%!ÂÈg?Þ®Î+"?³ZD®«…?ÐËPºœbf?°bUÿsº£?Ñ/­–•r?±òWiiM?Ä°Mmϙä?¨pëÞ1t?Ùty…æ?µó'Kô"?Ü3`AU­(?¶YՇ9"i?۟>è%ÌK?ɯüœô?Ñìiâ­ñ?ǝ¼{µ?Òtº¯
fƒ?ÇE¦IÍ Õ?áY˜ø‰ê?ËÏÖ}Ú?Ïí1saîÕ?¿èÝ8|ô?˽h*á«?ÂTÙÐûI?äIF§óé?±¤Bþ5I?Ëmل7ª?«
P{'?ÃmÑa(†S?©*hî?ÔݾTÜH?¯èRDˆ?Ô¦ÈTÅv?­äÀza¤?Ö| í‹^C?­µõGyÃMIXED3FGL J1745.4+4721@R'±F^‰"@>n9`sÞÀ:'ó²ê£À;Í
ÌÜ­À÷l–\ò@ªõ «†¬@wàyQû¿å`üŒ&¿éª¾UÌÌ]¿èHˆ&w'¿¨'‹‹ïøUNASNone?ïû¼¸=Ú½?5ßJê¸? Õè÷'?!\Ñjªé"?9¯²´
¿à?2X©?€ÝŒ?ï¹O|?ˆÛnԈ¨½?k·¬Ìs­ï?wo=¦#|?u£$4û"ã?ƒð¢Öã]Ô?ïL«zC?~Ñ¿xÄîw?C3kh?quD[?Iš¥H©†?v=b°ªŠ?ï÷˜Ò85j?XIü<—Ü
>¢UˆÒŽåL>¾‡5:(õ‡?PÌÖI¹?XIç=!X?ïýØ=ÌÇÍ?)"Ÿ
íiH?|";é®Y?ÅÓ:?g?'½Ý! 1×?$G®?ïåëéaqÏ?i0Q…D6?U² ªp³?SÕ%¿äd?^uŒ[±ï3?cØQç.œþ?﮽ÛB[o?m‹ç"C\€?ph£'ùº¿?a~½Æ3_?x8nçUm|?eÛ‰ü'?ïÿ'Œ7? '–ù}Æ/>SösÑÒxl>k"§¨7ï?Œ‰ñôå? 'P_¸cAGN3FGL J1746.6+0433@="¿¤Æ†@0}­ÙÂ~•À9œ-~¾LÀ;*þ±KÀúð¦ñ›ä@
{«lù¨@Ys_ÉZ¿åÇ\R׿ê¨Üäá°M¿ÚÖ\j[Šã¿é–è4l×UNASNone?îí@gE«Ó?£N Ö\•?y@í¨³ì˜?òœ~µl?œ·¥
u?¡©'î±L^?ïX=¢^?¡ÎÜ'þò?sx¬üG%?|¨¶'"Ý? ´ø½
? o	Þò?ëtä×8>>?¦ÞØÙª?¦Fdƒ]Å?"µctÍ?¹5§™Æ0?¢a<L_Ê®?í2ìWñGo?­fùN?>£Æ§àÆ?D÷øO´\i?¶J€œf‹L?­žzÇø?祈P²—d?†ž"ØVŸ?hÔÔQR7m?l-ÝYÊ
?~Îmw+úh?'·™­è:y?ïҘjçÌÐ?|/F"æãÄ?[ðs¾?XV]«?ooTœŠÊ?y!JÈ>?îkp•®m?"e#s·,´?"•ß m{?…¿˜/+ÿ?žüÛkÄâ?Œz¦ÆE"?ïyçïàE?cÇÇ÷?¹ƒBFˆv?!ƒwç•Ât?›ö	|ā?¥VkeŒAGN3FGL J1747.0-3506@v.cÇOµÀ§|{{¡aÀ8MRÓâjÄÀ:²	Bžá?ãšÛ—&3@ª½ÐZ¡@UÝw"q¿æ}"®î¿éÀ¬cÜÚr¿æa¶DU¿êaé©sΦUNASNone?í¤"±ï"?°ÔW[ù©c?¥"AP/×Ú?©Î^°*"ë? "v²ùaâ? Ù¼˜xç…?×¼î^B?Ò1÷.M"?¤›Ôø?¸rÃÿº.?Þñš'š4?Ð/L äÞß?ã?—YÎ?º_kñ«v?ÇðœR™¼?±Õ_FÑ9ˆ?ËSéOÿ?±W'É?ÙÉç>+ùr?µ—Ë•–ô?¸á3'0à?¡±aýŒb?ßýËø'vµ?¶rß
Ú?îµXh¦ñ?ªb#'Ê8?œh¦o†nÆ?§;ëïuðÒ?‰Ø™9M?ŒÞF=g?ä™s+ú7r?ѕ3I¿£?·ÕŒ¤}è?³m\,ò>†?Ð׶¦«â?ÌiV¡³°?ê÷¶ùY{O?¬ûö2M?´q÷<ðÎ?¤¸	l÷`Z?³ÐPùûU¸?¡#jüîÀ¢?ä!þ¢TK?°sµ,½»?²\ʉ»%?"®S^"ªb?Ó&«`"g?¯Bd
ïåMIXED3FGL J1747.3+0324@<›0aǛ5@/—Õ#³coÀ9iRÍ,nÀ;âµl]÷?¿€3¨4MK@
ã¤)Àn@Õ€ÙY¿æj2X¿âZÍÖâû¿áb¾Mz~™¿îWÂ?'K©UNASNone?ß/Î;"1ö?Éb"@?ÝŒ")?ÈÉË»Èb?­*‰"?°¯π¬?ê·Í¦ˆâµ?À´ÀeU?·¨üf'ñ?±ÜP
d?²˜–e¤Íê?¶ç¯ °Óâ?äcä–ö"µ?³¢†€u!?Ët:'q/?°Ó;ß|?Âü3!•{þ?©§uja±?àÃju¥Û?¸êȌ"z/?ÀƺwhIô?®Z$ŒmÝ?ÖmîM®'?·ÏOѕ±?åͶŒnŽ?ǯ¢ô¥ó‰?ÒZðHtZg?ÆDõ•h ? ï¢OJÀî?¬UUÓäF¦?î<'§"`D?°"(ÝÃ	í?žÛ¬ ?œ‡Ð	v¥?šÎÏl xl?¦EšZ]f?éWšdÎ>?¬*¬÷¦\y?ÀÍUj·ü(?¦*Ï^
¸?³¬ÈVû¢>?ž© /²`•?çöûàò¯Ç?¬½}¤q?²"ÅI#I+?š÷=Hü?Æá­ØH‰?§é"žV7‡AGN3FGL J1747.7-2904?À&'j(¿ÞZº LѕÀ72_½‹çÀ8í¸_~?ò«Ð}ÜO@·ýÊñ€`@ ?Ðû[¿â'†Là®V¿åÐ܎¶¼•¿æƒú¢Ý÷¿ê¬;ۀøAUNASNoneP?‡#çòµB+?‹/·Sµ"?Ïõ¿°ë«ñ?Ðw»'Të?ç¦s~Ž?Юhe;q?²21]¶?º/T8]áÕ?Ä__Œ«?¼E¯³G¦Ä?è·¡üXor?ÄX=iÿo?½´Ó8»w?¦8l "¿?ÖIîÒlZ-?·±Xv2?á$x›ÙK?·|/lÓ]£?¢sÀ€³û?­X›b¨þ?œxß{{!?šh8ö(¾?íõi/Þ.?³q"ÓŠjÍ?~cJ«1Šÿ?…çi·þ?ÐܤüND²?єµìWùÞ?çTæìU¹?ÑÀ=‡Êå?·F=pá°?À•Ÿ±?Èؑ´Q?¾‡:ðA?æá
íÃ+?Ƈh6´Å?Áq‰«Ìf?©^{•µz?Ö0Câ$o?µ'—fNîš?à‹•óëï?¶NÒw»á?œOõp}Ê?°ýøH8™s?¢ç•QÀ¤ç?˜ŸùÕðÕ?íïcî£?µ;M6H¨OTHER3FGL J1748.0+2701@IêÊÿm3	@9\gßã*À:H—hfñ§À;ˀ
|ZÄ¿ô=$*ך@
֛	Ü!Ô@8Š`¿Z¿åùzíSwn¿àC8P Îº¿é¹">o¿Á¾ºì¶³AUNASNone?ïº+qÀ.%?ÛÅášþ?nzJ%íjF?pÝė Nô?s­" 0?yÑü¡x£'?ï¬
÷"¢?‡öÎg§e?pÅ7i
3¿?x¤â{ted?y5Áx{?€‰©Ù  ì?î	ÝÃçš?˜tÖÊ/A??š>9oº?ŒdrHÜc?¢Cžš?+z3ÿ?·?€£Âú}j}?7¾>—>]À?AýkRc?ˆŒNðb…?€YpY8?ïëÓE6ëÏ?ny/êE?PƒvÞ«áä?]H')µ?WÕþÔx¿?dÜkv~¶?ïᑔßÂë?h©J2ó?Yt:,~:§?TèŒBuö?a´MöÀ'®?bÕi"il<?ï@…ƒ.ž?ñ¶`®§W?†¡¹|!´g?x6þ.B­U?‰=c¤?uVT!¡¯¢?ïð¦?^(™?SÄýÔ?§²pŸ›?)~TY†.?]öC—/Ù?S"_QUÿWAGN3FGL J1748.5-3912@u÷ù=ÙcÀAhr° ÅÀ8סÙÙû‰À:ø
ºÓ¦?ðofÈ61@œ4¡rV	@mŸ€8t'¿évq¡Wþð¿Ñèß	Ü5¿ç­o÷¿ì¨Ð%Ǻ¿UNASNone?­JöWçpÞ?°{‹G¹€?ì~?Oîw9?¹Ÿ¹-ފ?ªÑ¬ ·?®˜<î×?ÂaåÐKSÞ?ÀB(wv?ÙCMÛ]¼Ò?ÁMša.‡í?݋¿=yý?ĜÀ¥Aª?Ó2¥­ôù?µ»~û‡?Úî8~ý0?¶Yû;»'?Ñß"j8-?¶–ë>G ?Ò)ä{b?°+¡ÄÎ`'?Ýt
Ìyô?¸…ì	³E?п"àO
ª?²ÈhäË?¸øuc'¦ü?»>m	S÷à?ëGp¬æ?À­®f&Çâ?¬. À8¥?®3Þ~Ðë?Õsèß@܃?ÉjÎÕæ{õ?ÕJæ=¾ä?¾
";Ó.ª?ÕA1dš?Âg9™˜†¹?ág§Ñb*?´¨o=ƒ å?ÓjÖlLž-?±iMG¯·«?ÄÌ´ˆ!:ý?«E%ƒZ-—?àU`ûK
?­— mÖ?Óþ½vÝF?¯]ü•ª[:?Æ®^•À#Ð?£‡‡ÂX^úMIXED3FGL J1749.7-0305@6ú¾Yl'à@(o:¼"peÀ9,AˆaÀ; ¡`7x?Æëñ•®þ[@ß9Xç!ã@fÀ_ñ¿ë Þ®ÁÊ¿Õ@ÆÚ'w¿ç‡½;èÁþ¿íË !³ƒûUNASNone?ÚS>µóB?ÍñBÑŒ?âOæ‹ÿl?ÍÏ5Òõ°Ç?—dAil?£ÚRp6?çƒ>Ì¢
9?ÈíÌÄÍÇ?ÀkÞýÉ;?¸åpõ?Á‡øîzà?Ávby?ߺ-tq0?·'à%n"?Ò{"°\ºÒ?´=¯'8?˔ÂD]§ü?³LJ9˜«?Þ²fw¶Î?¹Z¨'/ó?ÎKŠ—óý?º(´Ù?ÒÖ§Ô<O3?¶ËK²ŒØâ?ߍ'ÌNUV?ϺGì?ÞãŽ'Âß?θ§òo@?˜õ
Væ®°?¡÷yë"??ìÆ
´"½¦?½39Žþ`?¨Á˜$õ8ï?¬p¸Zí?ªÝŒ'¹?²oðÒ^?äβvñ_?³yÓŤ?Ëß½¬ë¨R?®¬ñàäy?Àè‰8'2?ª'¿5Û:@?ç§ó퀪?«Ár>k3?¶:ï\U?¡âñ@8n?ÆC&AŠL?§ìpM'QMIXED3FGL J1750.9-2220@ö>¶5@ðï ´«nÀ9³Ët9À:oóþj¿ýQÃI@eÌ@AþíÜ<@¤hŸÑ—¿æ6ÈG'¿íáÇï~Ž·¿¯¼ äôXN¿åO¥&À‰UNASNone?Ö\Œîª1?Ñ•µ*ç?rè§ÞP¹É?€¼ž2í?ä¬$iÒè¬?Ñ0<$ë¿#?Û·TÿÐt?ØDù'ãbª?¡ÿôĘ?¥ó×ZrÑÔ?áV3ñҞ?×C¬ò*Ä?ÙVn
8ë?º­,«Qx?¸Ì8™4Ö?¦±›tg7?à;Açxl?» '°Ñ¢'?é…Nà|›Ì?Ãsǀ<?qZÒÅU?(w"`=uü?ÉçVR"nÚ?úCæ½?ÙGJÙ^?Ò»P99˜¹?t&¹Æij*?~źWS?ã4
K*"?ÒÐë7úuÛ?àÏ{Ïóâ?Ù£,,?¦"w0c?ªñ•"zà?ې…Ñ2.ž?׳]+‰q?䎢øp?·Gõ*?±‡e'3¬p?¡6©»y?҂V0')?µC1®ê2?ìËé¾êG?°F_
ד]?R§Å›¥Ì?^ŽÇÁ–÷?¹™â¥ã:3?°DTt1¼LMIXED3FGL J1754.0-3321@vQú¬Ùè>À'å=ÌÀ8çj"ò¬À:·D[y£Z?ò¹ÊE
@­\7äH@K?ëÓM¿Ëý4±ëþt¿êGVù'¿àÜÔ2Wý(¿ìý‹UNASNone?ä">)Ë?Æ+éþ5ûe?Æ~ÀΆ—?ÁuÅKpŽ*?É:î;e€?ÁÏÂJ'ËI?Õ
N†BF?ÑîÚhÁµ?Ãÿ™±J?¸7ÛÁ¢Æ@?ày˜ljXÜ?ÏHm"4O	?ßþ'Hš×?¸'4ähi?ΑöÍ|J(?²½qfc{?њù@?´š9ñz?ÛeÜË?¹PfûBÉ,?»R08?«ŠZ±XPo?Þ3αê?¸ËQ¸'?é¢üKëeê?Á=8\_HÝ?¹^L}¼VN?·ïà³Ø‹Ò?¹‰Ñ#Vmá?·lƒHwҚ?áË¢þû¦³?ÑÈ~MQ±<?À]ìá%…‡?µ"]Ç:Ï?Ô9Ñuï×?Í+\ö·=*?æ³Ó€‰ìí?±]Þ´—?č݇~Ü?©d‰^¼b—?À¢ÔîPÍo?§;)ô0™?â´E¹6†¿?±ûñ¥	¿e?Ä''cO¹.?¥‰gÛ!‡?Ѓ³[ëì?­XÅÑÜMIXED3FGL J1757.8-3126@vsC•Àv€®ç	À8ÞæïÁõÀ:¢MùÇ?ïÝæ"bè@
6ÐfŠM¡@[,å¾`?ýGªí¶ž¿é^¡i5Š¿ã¹ÛGR¿¿ìÔ°Å@w¦UNASNone?¬Ox§['?§ëÿÈ»¦?ßÞÌì$?Ϻ½Jù£p?ܗùÌ4KŒ?ÏøMŒ®W?µ·Ã¶"© ?½•¬"áº?×o˜íTà5?Â/썲[?á';i}â?Æ؈ººä?ÉòSÀ­•á?®uk<¹?Ö4)F\?¶G*Ý|î?ÜÒ¬Ù³?¹Œz•?Á«‡©hTä?ªW`gˆu;?Îf20v6à?±ÃÚ.
ˆ?ãû'‰ˆ]?·'¡¯eÿ?·•R1,2?´±¯eìˆ?âTÈP³™?ÎÐÐv"J¿?Õðã¸A?Ìæl}y?ˤnMªFª?ʛÇųF?Ö0|á
\Æ?¾}íM1?ÛýKøå?Ç|ÖÑn®E?ۖ=~»œÏ?²ÿt6U?ÓLqÍÁ?±bÆêLÉä?Ðêv:v/?°¯þyèÛ?ÍpùyO!?±"—ØV÷;?Ò©žº?×[?ª!&¼
?ޝ佁?²YH!«1MIXED3FGL J1758.8-2402@á•a%´Å¿¦7½D†À8c˜¢ù"¬À9æ×5??ðíäI–!@Yi}È?ÿæÀ'¢Ü?辶ÈèLì¿ç&k
·p¿ÑgîõX8¿æžºM8UNASNone?™»O‹~Z?¡öC}§?'ówCsì8?–|åü17?î¤fk'?û?¨ã×ñ½â?¯
Dï¡¢¢?º}¿ÀÂë?µÝúÖ?@?¯}t@‹äº?ëSœoaâž?ÁÉkæ¥]j?ÃÎS³cù?­.ŋöÿâ?²uÅ°ú? 	Ãx:N?èÉ-ɚpã?°¦JG-p?ûPÛ\)?½QëÜdù?˜ÞO"z?˜TØÁÄþD?êJ9LÛX‰?¿Æ‰‰" ?ŸŒ'±—?§ÿÚË{¥?¤Ë <où¶?©´È]Í?í¶íçÆðŒ?µ/ϸìæ?À?±í^£á?Èok8ÄRç?Àoß{Ó?°GG§´dv?çè7Œç¸?Êß¡Ì?Ë-ä²Ð*?®«*Åä@Ö?²üáÛar?Ÿô,œ+?æÔê—ÛJá?°Ðü)4@?ÇYî]ìn?¿)ôyÜ?°F Ób§»? Ky6]ñ3?è ÀMý'Í?ÀÎa%ΊOTHER3FGL J1758.8-2346@ÈëÌlU?´Ê¿_»ýÀ8^@'7|À9Ǩ§b°?ó›÷Aë]@
Üçl`Px@£¬ "Úƿ©ço?ï•ç·B¿äï]+»Uè¿ä&VÅ£RUNASNone?Š
˜SV:á?©ý­.:¿³?°$Ãï?³•Ü	{ŠØ?í"S…ýÊ5?¸ š¥[?³S]§2Ò?Å-W©+ªJ?ØK7&îèg?ÉÈmÜ@L?áoøɳpc?Îzø›Ôÿ™?»a®4 	?¤öW_¸Lb?Ðàq)íê?·JLÑh2±?ä#'¤¥Ù?¸p>)d?°	NқÏÇ?­Qƒv¹¸?â²¼¢ª‡?Ì2¤ºVtù?×øFÒf- ?Í1\¯®Y?kØînF?r\z¬ÿßí?±)ÿKÝˎ?µÝíÈ¥2Å?í¾ç(eZ?¶^ˆç
Îq?¸Üv'c(6?Ç»c$ßÕµ?×g—Ïüq?Äeº•£Ñè?á0¥GÞÍ?ÈÛÕ¾_æ?Ã#E™+#‰?©KßA"?Ïf°™)?³Ë'˜§ö?ã]¨­'PÓ?µzvÙ²*¸?µKïÍÅՔ?²QÈLD7?ٙ¤€AG¸?Ã0[¶ùÀ?à‰¯Å鱗?Ɖ'ŒÚùMIXED3FGL J1758.8-4108@uì²êòÀ ÷W÷7ÚbÀ9Ÿ"!°SðÀ;OrSÍÝ?ð9ýŒÞ[@¨¢?¢§@ÓÙ m2Þ¿ÝÔR}%o¦¿›÷Dg"¿å÷
€û¿åm|^ªöUNASNone?î's8ñ? UIˊ‰Z?—ø$öÏ?—.Ø9û>ô?•ÙˆËTÍn?øNþWI?åTqj'?ÐMz)ÅSå?¶š5höP?³Ú‹B½	£?ÏbŸ‡oJ'?ÊDêÉ?­?ìD3ncØ?£Ž¾M¥?®ËÓº"?™:mƒþ¯?¬ò9cì?—$#ÉÿU?å¬ïŒÀB?²(x'm¨?ȱëÞ=–?±SÞ²$c?Âç`chá?ªƒ†4q}š?€‹oy?‡exˆZŠ™?wšP+Ç?€%µP?A¹?~3%uË(F?wÉ쩱u?ë'6æŠÓ?Ãeò3tÝ´?¥xŽÿY3o?¨zâF?X?¹2ÆÊhê0?¼™]xoí?î'v€›?'Óç
²ô?™¬Û]ÞU?Š̃È?"Tœ'%?‰›@Øù.?êçÐBðaõ?~ÃÚ~ÉÜ?ºn2ðd£æ?—l0ÚÝ>‡?¬¦•ð0˜é?',Ì3þƒAGN3FGL J1759.2-3848@v0@9«óÀ´ãy·|À9qiiP%²À;ö¬š'^?ôÑïK|Ö@×ëϜ`@ãéÿ"S?êužåÞÁ—¿ÞWí',Q†¿àRcz¬L,¿ïÿû)pU—UNASNone?°³q=!L?¹ýìÄ'Ño?écQ¶"ˆ¸?ÌnFsp©Ð?ˆwC•?Ç›ó; '?‡nfPq%•? ŠãM‹²?çg¹0$û?Ãë3
ã1W?ÐuNJ ]?Ã'ý³R0?ǃ2Ô,W?«®"Ž©ä?ã"r_1؄?¶Gk"¨½?Êk¯™?°wz.÷²?²Ó¸·Vô?¡êÃfxƒ?åÑ/Ò?¿åÃ`3é´?ÏQë3ƒÿÃ?ºûZ˜–©?¶I'ä&cJ?ÀÎ¥ƒÌl™?éO¬1H?Î:l–óø?¿=¿ºPÚt?Ç#5qp÷?š½ñ4,¤Æ?¦÷ûÍáã?è"øBòC?¿üZ]ÞF?ÌÁøn¢[?¼Þ<`Ù^¬?Ù6N¹ª
ä?±Í´ÂŸ?Üðê%ç?²‰~
^þ·?ó.¸q˜k?§ ïÂäo?õÇ&?¥ÇGߊ)?åK*ez?´°8ÿfWA?ÇÀՐÉD
?­¼>Ü µPSR3FGL J1759.6-2141@dÁr%·?î¾UíQÀ8ªO¨´¿À:0``'çÏ?î4)¼«±8@ò҈"£Ä@Ks«¿ìMÃñö—¿â¦â+]¿â¬Ö²°¿èö® þìôUNASNone?€N¨ÞÔ·?ƒL¨däŒ?¹ûÓ0Ð=¬?»dJ©Ò¤?ìKc˜?¼Y6kæœÆ?®˜~b4?¸!ŽCåç?lj•ao1?»¸ë!)N?è4×2Á?ÂÑnß?Ǖªîøé?«­§H§æC?Ì¡Mhϳm?²+ì_ª®—?âòAé"h…?´ØR‡ÌD?ÀhDµÑ?·KDUë%?½qõÝ÷?¯àºÈíx?è7ÌÜ«ÖÍ?À°m#L"?~…-'9œç?ƒÕSnfù?¶'êZ<¼"?»çA(z"?ìð˜Y†6Ä?»æׇ]N\?Â@ ïSH?Ãhº5'ÖS?ɇìöuþ?¶¾"•û+9?å
ü†½®?ÅÂ:­PÐ?Ñ;šÂ°á?±Æi¥Bì¥?È´ƒªÄå"?®S|í¦?á5³lå˜?´tÔŠx?Äh$e©ÁÊ?ºg4¨ºZ?ÆDÈB4¿?©>‰ô"6?åTÄÖ_Ë?¿èqáø5ºOTHER3FGL J1800.0-2955?çò–öQ*•À	¼©ïR2ÓÀ8®ñ7æ [À:k¹8›R?ò¦©½S2,@Å2™Û2ì@N5gÙÙ¿Ô­æ¡Îá¿ê²ÞŽ~ˆ¿ë'ÏÐã1é¿ãʎÎ([XUNASNone?Îôå\]…?ĪÓé Àj?ÂZâ
|?ÀÀ=@ìóø?ã¬Fð6?Ë¥¼Tº?ÕЫÁá%?ӓGö8Öá?Àì^¯Ûç?¼'2 nÓ{?àܒ…(Ht?ÑãDà|#‰?Ð7§Æòi?¸1ªX±?Äâ¼×ç?®H'Lè?â«} Ò?¼¡Îä¡w?΋ù¯;]?º	°¶tN?¿'ÉoäÙ"?¶He?7?äjÈe´å¥?¾S×Ìæ÷?ÛÍزÖy?ÍÅôÇÎÇ_?¿• ò×+?¹ËÑûht?ÜýÊ&s¼?Î[O†ûÝ1?â¡iLçw?Ô?ô§‡C?¸)¼–¥œ¨?·Àvƒ¦#|?Ô²¾B4FÈ?Ñ-é¿L?á(­´¿Ëï?º1ã<zڒ?¿ˆ§Œ{?¦ù>eƒw?ÕÌz³`¦D?¹M£:ø¼?Øt¿ì$çý?¹˜˜2ìZi?ÃBïË¡Ëå?®èç…(×?ÝéÈ.
2?º­ÊAñ×MIXED3FGL J1801.5-7825@sµ4'¾‹ÁÀ8b{öÀ9t¢ŸÒ™À;?Mó¨Ú¿ë)Ԓhø½@ó*ÁŸ@	òŸÅ,Å¿ê[i1¿7/¿ç@.·V §¿æ
Ðl-j¿ãOïáêtUNASNone?ïý a´ÐØ?/þþˆ­Í?Úfzµ?,2dòF!?.4at",?-[^«ÿÐø?ï~B6õú1?Žcûâjí?läw zë?uƒƒ'ÒA?‰6T~F&â?ˆÎÊäüT¶?ïž°&E[?ƒ×dՁL?ƒo'o£ƒ€?quÍå62:?"ô–IÀÙÉ?€¹*ÚzZ?ïÿ³Ã«*??½>C+?6|Z'}&ì?6)Œ¯Ï˜@?L00ÿ2?2´ —£?ïþƒý ?#ت"Ìu?	"6õµâ×?xúEÒ¨?!m'"\Íý?"&­Ÿ™o?ïÔé$W‰e?pO–x¸[?UÏÍXqñ?R—[vªH—?pzšKØ]?jä#eÀ»%?ïŸ=W¤V·?mM‹Ö7ܝ?sTsIÏ?`•%Ož€?}ZP½4Žà?f
Í8N›Z?ïçýhAÞ?Z̦¿ÐmŸ?Øù–eþ?4Z'*B?gT#ÄYy'?ZŒ&Íæ»AGN3FGL J1801.6-2213@uw¾}~±?Ó|½U`"¥À8ÔQ ˆ6À:1sˆÙ?ㄾ2Ö"@
†ÆÎ[S?ÿ{vÁ'}?ïò"c"'¿Õ89Wd•×¿é'L"5à¿ÃÀdÿðUNASNone?…`	øHÈé?ŠñA~Ù—?Ÿ[ˆe4z@?£¦»5º-?•,2Ê?§'fLm¨?µDü×ì
Œ?¾þC"¥®?²TóÊ@=?±NfÿKc?ëÁ냂g?ÃzŽÏĬu?ɏ«ë<	Ø?®f>PÝ8?»ÕcÎu]>?¥Ê³9u9
?æ!h‹bQâ?²uÙ$bϝ?Ь%3&"4?ÂnåJ
ÿÒ?¤s°/©m?©x'sÅ?æb²e©Ž@?ÂXËûÓ?‹˜·H5‹Ä?—§m}?èAŠsgÕ?7uéåW?ï
[bSC?¥¯ŒüÑm?È|¾9¢?Ï(ìMñ{?µæø2O_?­àùEúÖ¸?çAŸñ]¶ü?Ð!|UÕ¹I?Ñ>sâ‹6?±Ï•«­«:?¼óé`5Ð?¥'öV=aP?ãÂIG‹s«?³¡ÄܲV?×ðîa"f÷?Á½µ§0ð?N«™'W(?"òÔrjÂ?ãr^Ó[?Â$=7÷OTHER3FGL J1802.4-3043?Óqº™MÀ7%_5½À9?»vc3¬À:ÞùN59?èÒD–ï@
}XsI@â°À|²X¿éþ*7Œa¿à"…‹ð¿Ñ2©gR»¿çy‡‹ÉDUNASNone?è×°æ'E½?Ã7ñBàg?¡ùT¢-?£úFÍVÐë?È"ç>E¾"?Âøm©?™?Ø*×L¶?Ñù×Ìc?"ñá{§ä?·?ÑL‡nÔ?ޜ\6â•6?ÎÈ­Ê9ZÑ?æ C
é?µ#¹—H®?²bŽ?žQ?›!ìÕNþ?ÌóM¬¨Œs?²Þß÷[r–?àžO´Sx?Àì%¬õR?±ÅÏRo+?©ÿ¸
[Ô?Ú~ï$̤D?Àó"Aî?ëÕ–ûÉS?¹#Ä£¤?‰³~ɾãF?‡N˜×aW1?¾!3kè0€?¸NHTBýu?äF6õNe?Ñ.×{Hî?¹,°¿¬i?²8¤¸xÛH?Ñ(fcä?Ì9È£S?ì8µ:è?¥½JB?¡`úÒG?­ýaLô?µ‹üU¯¯?¢.ËÇž<?åyîºZë?µÏíè3,>?»pm•¢Â?£·âÕ®ºì?Ì`&‡Âñ?²\š'‡5<MIXED3FGL J1803.1-2728@	ÄÙÆ°SÀ³#»ÆëÀ8õ	¾ºÀ:ŸŠÙv0?æàK£R¼!@0î™Ñ!ñ@°yݽ¿èBšëdx·¿ãðd@"»V¿ç
zÎ
¦¿äâlÊ갟UNASNone?è^ŠË†·Ñ?ÅèþíÂw?½¿Ö;­Í{?¼‡'Y¾ÀÎ?¿KÓhsÿ?¼n§×¹©ž?ÜìhØufM?Ó¢d¬°€D?¶À×U×?³3È[-`?ÝcaRš?Ñþ`úQü]?âřÍFj?¸fyÛ¹?Å`ß´*·?°œ-Ô(՚?ψ¹âo¡?°ò^eÕ¶š?ÞUƒk@&?¿"$'ÉÑù?ª£TÞrŸ?Ÿ¯?¯S¦V?ÞVÈ*ÈøÏ?¾ÇòaJ·x?ííF¤vŽÊ?°3|Qôº3?¡÷®»iÎ?¥¤N×¾V?ži"–‹?¡Vðû…f?çÝ$UAG?ÐԅêBæ?ªMgÚãC?©%Òó8?Íe1y
½?ÍaýòšÍÝ?ê°¶ÄÖ;ê?«ËŠK€®}?²Ká-ٌa?¡ÝãŽnèø?¸.h©¼ÆR?¢}®¤À)«?årSá?µ?¶ìi3ñ?ª²hNqGÙ?'§‹¤ØIÕ?Òu€T³ƒ?³ÂUœíMIXED3FGL J1803.3-6706@tmã}é9ëÀ4^,ýxÀ9†‡OêùÞÀ;§âïÙ?âÀƒ!w@ΰýŽa@»_ÛÝ·¿ãâ݉¢D}¿á-0K'Ï¿ã®1]›¿éí.ÔßôUNASNone?ì}#¹‹#?³?ÎO˜iz?°zYæºÚh?®/Éy¿?§9¥'4ö?¢77g÷?èÇwš¸ ?Ä×!UveH?½ãPò¶ÁH?¶A)£KûÕ?ÀÃ9¨9¼Ý?¾<^ž#Ÿ ?ë¿×:±N9?¦*l‰W?±aקWƒ†?Ÿû°tƒ]ä?°Ÿnƒùñ´?—£U>§®Ñ?滂1ÈúÛ?¯'«$lT?Á–&P)k½?¥ú-ÕX¶?Ã{ÐæŒçZ?©z3"­G?ï(Hõ? Ë–¸Zþ=?‹âõŠ½%?Ÿ[x?ŠÆ5Æñ?"4fœf²w?í ù¾âQ?³¦y£pb2?¤àºj>p? LÏt¢?©©ø(Ɍ?¬)ï¶?î¾
sÓXÏ?Ø`²?–G¤tã¤?‰×ysëQv?'ö­	Ò«x?y"É_Ü?쪻Š&¬_?—™y{PŠ/?¯	yÅK ©?Ža$bSêà?¦J͜•h?GŠ"ñ+-AGN3FGL J1804.1+2532@IÕcíb@5*ò¥¤i×À9Ä*lEÀ;˜€LÁy²?ï¼ú@ÝÂ2…@µŸe`'¿äë]ÃÌëM¿î›"rëÚÚ¿Â5¤"ÿY¿ïÿÓÉ&‹@UNASNone?ï@¥ë>.?Ÿs$¬?uÛb–=?vʲڟ­?'¨¿F?œn"Þ#Y?èî@©­'?ÊÜ&$?ǐ©)žMÍ?ƛ²"§tÏ?°Ï;¨Qâ.?°Ïú‹™H2?êhÄ®´øŠ?«†M¢|?µ0Ðe8—?¡
¡Ó0$?·‰
%(ö?¢ëGTZþ²?é:ÛøR¦Z?¾˜.N`Ïè?¸ȇ	3?¹E[2Ño'?¾ Wµé€?²HCZ¯'?ï†MD?¤H×+ÂÉ?kuÔÐý•?nAÖLÿ¨?‡žüïM'?£TÄ9–©Ä?é6½ºÇLì?ÊÀÁf<J?ÅKoÏ	¬Á?Ç4B–†?§fe=??§ëZtž@%?ìübÍ»ÆP? þ"26?§F$Ÿ:.?"Æâ?¨ó¯«Ï?˜ËÛQâ?ìa|IZE?«D1Q>ˆ'?¶!IîääA?¨7E ù'?›Z(»A&i?ÿ_î"v3AGN3FGL J1804.5-0850@3¦Rz WŽ@ôº"»äGÀ8¤3¢Ä»†À:¿b֎í?ÛÆ:{?Ö@§!lŒE@þÏ@šyé¿ìâAa&ê¿âÅÝCVZÄ¿á"
ëiß±¿èÍ/UNASNone?îjý‡TȄ?ªëÖfZ?•"—î5ã?˜3^ò˜}??{Àë˜?§]fŠ?êì`Än?ŋ²nZYE?£ÍˆYabt?¥Cï£Ni¿?ÂììeL±?Â-顈•)?çÆØñÀ™…?³§ðÍǙ?³_;N¦Ë?ŸÆ,«¡ÝJ?Ç4þ'S?¯Á"û{¸'?ゑ6Ú÷?¸±ÛrÁŽa?ªJñ-
Ü
?—yºÌ²/?Õ±Ó¹"Ð?¸\5/î¢?ïwnÔý{?¼îÅשä?u
Uˆ§?™Zž:ח?˜OÎ͐ë?»'Ì&ùWß?íÕ[Lèø
?µ¶É)†€?'äÊÂ?™>G:0\?©[XÎõ²N?°v÷Õ¥h¤?í#ôb#?¢ÉfÿQ"?ŸóOÖG™?¹cXLÅ?¯ÿ"_?îðD=u?écêci9ˆ?ªÜV «Ã©?¥tn¡OCÖ?‰c,›?Å:Ë¿è?¨ØA(¢=AGN3FGL J1805.9+3407@NGæÿ}ú@7¦êÙ'N#À:µ7"Ñ‹À;£Ò$ûb?ҜkÒGFL@3úkU9@Êî «†¿ãå~'*ð¿á©›yÙ¿ë‹<7yúÿ¿ïüO¹ÑlUNASNone?ï%%Sv ?½Z$Iòy?š¥—ƒÞª?œóÞéÂÂV?b®tÖßÕ?eÚó¿Ÿy˜?툐h -{?±›mkS»2?¦'Q-¾*þ?¡W=°bÿl?¡O¨P>ýY?ª€	2€F<?ìÔøéœw? Áo]œBŠ?°ŸhD6/?™ÕŽ†MÞñ?¡q¡Q·"?Ž«©3?è±ÎL\?³98N?Ğ­$ù<?²2Eý"2?¶2xLgæ?£*-®'d?ïŸɋyÆ?ˆÍóhlû×?…÷^yŠ÷?ˆ*͚8a,?Rwß‹ô?Mšƒ®[¬©?ï?ЯÊ!?˜"â%Å#›?‰·a–5?‡‹¨
ز?†Š}Hµc?'æDÿ¿Å?îhÏoÇìœ?"%°0v×?¡ÀiDŵ_?$ј#ýÕ?ŽÊ~úî?~¶®þ‡¼A?îÚlakð?'ù$gÀ?¢…U×ÝS?Š]ï	s?˜š¾ðr?†ÉŒÌ7ÿAGN3FGL J1806.2+2744@K"BJ'k@5ƒ
®>lÀ:w`‰­"À;¢bAQ?ìßôi@X@!eIZçØ@ÆlZ(@?ÀkQF;¿í@Y?¿Õ¿†nª¾Á¿íÞES­b`UNASNone?î-/Ê.H?°b"6è¦?§åN
}•?­'࢟ï?Œ{Ôkº?u¶ª:jy?és·¸«~?À±"µ•+S?Áönìþñ?º)[)—?°uf1ØØ-?±ÄÌ÷ò?çæ\m
¼¿?³"#?ċs³x_Z?®Q|^Hž?·¶5-·²Ú?£½%¦1÷?åK}í@µ¨?¼¥[â²oÝ?Ä"¿Èµï?ºœõ;"b?Æ»s‹4sr?²ÀŒxæõ?î[(ßa?¬ú™q}1?¦Øb^ó?"?¨6Y[І!?ŒÇ¬>œNÔ?‹çw
2ï?ìò.aþâ?²KÀR•ùý?°É·`jS$?¬ÿˆ³X·›?ž"Vc­Ý?Ÿñž'Ó?ëTY7÷	¯?§´Ö—îø?¹œÍ;î©Ó?¢ÿ›×•
?§€Ò®Ày?•'â)'…?ꇏíãÂ?¨"£×^9?¿£%…š¬?¥Ú¯-g‡È?¨@¶÷Ÿõƒ?"ßìw'¢ÞAGN3FGL J1806.7-2451@"K3ÚùÀî['ÍÍÀ9;ofÀ(zÀ:ywÞ]îÉ?èÞÎÆ2e@
×Tª1@«å÷1¿é–´~¿áP²êšàc¿ìÖ;Ÿpý¿¼ß¢-«¤UNASNone?Θĉÿ•?É=0¨ûrŽ?ÉøàôC?Ç8Õ¸ÈwÂ?â<þÛ?ЩjcpÄ?ՄݸŠÿ?ÓbÃv.Qï?´ÓQd£M
?·‰vãkˆ?â£&÷Xo?Ò¸±"Y‹.?ØÉüU?¶,=çp?Ëó"B	[?²°éËÃßÕ?Ù<9ojú}?µ€âCÕ¸?à|@õ,,?ÈyÄM]'?ŸN/ö?¦Ù¦ÿ!¢?Ý›#ÏÈ?È\v*ÇÄ?ÖÇþóX?ΰè.—?¹…(½´7?¼–¨ì{qn?ákÍèo"a?Ðg(þ¦ä†?áБêg2?ÖX›àU?®¤8ȸ.õ?° ½¼mìÞ?؊U÷½?Ô?ºsÇ?äkpp\a?µåt»5?¿ƒkã[?¨e®V•5?ÎÂü‰¨à´?±ËäíÆe¬?æbžÏIºð?¾øæEÄ°I?š/úЈq"?–ð'ÇyŽ¨?ї´šüÆ?¾¨ ìšÙœMIXED3FGL J1806.8+5346@Ty
®>lL@;ÿ:Þ"_¦À:#éõÒ"À;ÛzMÝÙÀˆ6Pôå@Ô(ú@@… =w°¿å«lˆûwì¿çÛ×ϊAb¿êy£¢†þ? îÒº…IUNASNone?ïûȔ¦7?@ºéÆÿö?,±Ùž1<R?-"üd%¬ª?8¨Í jE?<dÔG­h?ï¹ÏðÿÃ*?‡ZáÓ
?l¾yÝB?w¿C˜eµ?t¸ÊŸ+W?s
¢¶œ?ïEʆwÔ?€ÂÚ@ŒçÌ?€í!д2?rý0Í¿D[? >Bh¬Ó?x·{T{¬›?ïñgf@¦¹?_םóîÌ>Ú,†sx	>ítÌÙk~¹?]˜âÖ?_Ð&‡ü$?ïû±Ák"?vBôºû	?/éÀYpï<?j'«¼ÆH?2'kÍÍ+Ñ?b"ÒHwi?ïåº\»Jw?gDˆ'Ò¯?V*£ù4*õ?SË12Ò6*?^`¢z9g5?a~ø¦?ï¥x¯%c?qh[3,}?r؃6¼?eeêy]Ê?zk%"G¢?j`묦±™?ïþWá_Î>?-tšwD֕> Nqi>¤sUxö¥?*qÞÍ»{Ò?-nÝÜ©3¢AGN3FGL J1808.4-3519@vM—á2µ_ÀsV?§µ¼À9¤qJÅöðÀ;8ñ±ˆ¤?ñ/áo@
È-â¼MN@xÀ`'̤¿äñ-Çl¿á"ðŠ—=¿åp-ÇZêT¿ïýÁÜPDÞUNASNone?´[¨.á(Ÿ?³A.út?è2ºT¥Ü?Äý¨_¸ªß?ÅB–Ÿá?Á©|÷³'y?'Ž´ÒÛç?œ~=ûï
?å‹~"aÆ?ÝQA_?ÓÐíªxÔ?Ã,gK,'õ?Ù¼ÐÇ>~§?´V›@ƒjé?Ù •é?´8Ä¿Ò?ÊbEOb?ª>1…\k~?ºAL·¤Ù?£Õ		ӎ>?å-Èžžç?¹ÁùÁïÆn?ÎA?')±ø?´™8ýãË5?Áº2o­¦±?¿±ÞùŽæ|?çé&¨>?Æ9ñ#ªeU?Áö(õ±aP?»èY´ëô?²Y9dø?²©é'â<·?ä´[Ô^ˆï?¿<^Uí?Òr—9~?½8#D*¸?å¼qˆ-‹~?°øՒ Üø?Ì<MW=m?¬Ðx"A?¹£ÙŠ0¬+?ŸX ÇX–0?ʨ¥ë??¨êãÏwëØ?ãÑ¢ñ(?²"¬ÇÛ?ÆçÆo²ã?¦iETMMIXED3FGL J1808.4-3703@v52€ñ,(À `€ù£wÀ9ݛڼy˜À;^G;'ô;?òÁ1c$g"@Õ'X3¼@‡¿¶cÕ¿ÖáY«[Ò¨¿Ü× ÕË¿çKbã鸰¿ïÿmäñUNASNone?¶§VÓ˜?´s€i퐄?æRFª¬?Êâ¥Ë'K?Ëc:Ò)ƒ?Æ~ÃlVõ?¬"Úþ`?°Oø¿¸?ã›ažFÔ?Ä@b¬Ù£†?Õ6Á'Á»Í?ì]bþõ5?Ѿéô"«¸?²'"VËŏ?Þõ¢=T?·Gb;\Ã?Ζ眠£é?³â§'_û?Â,曈º?¨ìʟ9Û?å¼Â0h[?·öt€¤bó?Æà7µÎÙ?°ÒêC`?¿0h	¡
ô?¹îÀÅë?æ¥Æ†•8"?Çï©æ·ý?Åбàژ4?Á¶'Bˆ?ÊNà<œ?ÐÝ)ޘ?àe™Š³«F?Àé0·8R?Ò
¼úzb¥?¿ñ'mÅ>?à× |'õ?²ûnÍàj†?ÕÌ]f7—q?±!y
¼E?Á
ÃAL•I?¦Õ_Uk?ÓûÃäàƒ¨?«6ó-Êîš?áï†Z̀ý?±讽ˆ°?ÀJ^Í.¶;?¡m¥¶7¨ñMIXED3FGL J1809.0+3517@NýéÀ"š_@7aæÿ}úÀ:&Nw\WðÀ;¬GðY™Ï?±|a9L@
ƐÃ/@‡þ¡e–¿ä2‡»åc¿éÊ'•_!¿ÝÑnµÈ×Ó¿à¥R­29UNASNone?ïß\O]Z?oŸ)2IÅn?9ނ½uýÌ?7"9MîÊ?mgßÖsxu?npè îh¥?ïa½ÌÌi?™[.´OPÁ?€e›É K¨?ƒíæe!?‡*ðöK?"(Y7"e?íí´¾/t?—Ssýù?''MVVg?|ÇLÜèb?§Ü
m·ú"?"_#e°"û?íÙôJ•$•?šêø_a_M?€šàiØMï?~å@7ÝÏÅ?®:=Š5?˜³Ââ(®¿?ïø-zã?M–m%N¼œ?#óÃàCû?"ë†^xH?JOÚ/Bi?K5ǝýf?ïÊý£É=?|fg~Ƅá?fÙ?p)B?f–Ó͏C?n)Ö
áë?u}1Q"H¤?ïLÚ« ™l?z}]äE8??íы?½?d'Šý~)S?)^Rƒ¡?tµ.=Î¥?ï}Ϻ¡?x]{ùþ
Á?q¸î=FǺ?`Oc²î/?‡¯šMMڌ?tøK•ÿ€AGN3FGL J1809.2-2725@S*I¥ÓÀ	í9SÞ¤À9X*ˆiÆmÀ:Ññd[Ê+?ìJõA` @þ~^@x›_lw"?ïÿW'rúb¿ì>Úcì¿֡Nõ¿ç[k•>.ÿUNASNone?юt`龏?˸[Hœ?­¿@©/½?³üñU Îö?å_éÛ·‡|?΍î6v?ÔÒL¨ûz?Ò0½…øí?ÄÙtƒ"%•?¼#uÝʈ?à`|Š°Þ?Ð'>NU‰°?âVsb*ö?¶÷×'¹)?¼ì»Ìì¥?¤¸íU…!û?ÔR^¶ØÖ?¶É2®;Ø?ÐñÙ%œ?¹ÀH*õ?¸P²vÝ?±è²]ñ"?ä|ý)"Š?¿\
K[âÄ?Ûÿߗ2i½?Ð CÏ/?¦ëäN¥}É?´f@ȧa?à'Qï`öe?Ў¬~Bé?áÚ7rÌ¿û?Ócêt—Ep?À
ê2} ?¸Þ Ç?ÔDœ{?Ïý)G2U?éÑA	?¬)‡¸~f?®zÙ±~ì?™d¬Ïl¿e?Á؏	?¨€^"¡¿?ÛÉïíä£?¸R/L?Â÷R>]«#?¬'¸ÿÖÞu?ÚºfóÿìŠ?¹èà'ûâ(MIXED3FGL J1809.2-2016c@$]7qÁ
¿Óï]ŸˆÀ8)SÂóáÀ9¬†2´ˆ2?à¬Dh@
í÷ßõôc@›&@©¿ãVA`{‹¿éÞ)å¿æ"=Y|Èþ¿æÜuþ†GUNASNone(?`÷ge¡èÆ?eiÏ÷)Â?‹g)G©á?¢ãþPƒ?ïkóC.(?¢ ±	ye?°88s™?µçbÉOŸ
?¾×Ã\ðÞ?·}I™áo?ê! 'gµ?ÁNªG'¹ü?½îÎ>Æ?¤ïWé°d5?ÅÐľ‹k"?±e²?x}û?æÎ
×%¦?´•ê·"7w?´OhM:S?¶ÒB—ü?˜¢¶$Ÿ¬?';"[1
›?ì¸aú›è?¹¦ÐµuÔT?Z	ñ4¦öÝ?eˆ±XÁÑá?Œ\AìGß? ^ßÊ°†Ô?N"
? ø†Î‹ŸÎ?ÁxÓ6¯z¾?Æ
ýÆ%$
?Áœ/Á8Äî?¶%#Vðr[?ç:¿Bð?É)rÂ6¾%?Æζ©AO?ªŸ(r¡y?Ŝ€o¸/î?®'ê´‡–?ål6g£±?³UÄÑ*Õ?µ5òJÊ4?»ïYOã©C?ž^åróØù?'ÏƵA?ìfJ‹$Çò?¾¯£#ä"OTHER3FGL J1810.7+5335@Tq´ör2@;h}ˆÁÛÀ:|¶ýW¯À;ÞH'¶þ.?í&/Úc8_@
Ç«äÊÅa?ü{óI"¿ïþ§UCÿ3?ïôù&Ёì¿ÊÖøwG¿âOEèÂv³UNASNone?ï»Å®í¶?šo"ÓàQ	?i(Yïï>w?vaw×æ{?uép£ÉÑ?™Š¹ËËíj?ìˆBç†6?µ<¹=Õ¡Ó?±ûŸvÿðù?¯Û]~ù>Í?£"'™œµ?¥ûzH0ö?í˜*Ýèí¯?¡N
Àqv?¡"öÕk?"ä­™IËM?¤ù8zO­?—^4Ö°Ø?ë¦õ'x•¾?³ÈkRÚ#•?½TÙ
È°Þ?²£HrC?•Íë…Ê"É?"µ
"uËÜ?q¡[7'?¡µVyäf?]Ûk3ÊCÆ?cØ>½ü`?yÀT¡žr? ýgÄ;W?îìw5|ʽ?šïAìqs?•=°Ò&?'ÑÅ<Ýv?ŠfÒ|L\?ŒlŸO5ÿ3?îÕF¼ä¸?'thæ&Ê?'w½œpH?†«5,Åve?'ßjÈƎâ?†
0å¸òs?î,%íûE±?šFCBy9?ª¢e8q"?˜zjKŝ¦?tÜýêw'¿?t<¥ ¬"
AGN3FGL J1810.8-2412@¦ÚhµÌÀ2J…_OòÀ8Œ°±
S¦À:,ñ.?õƒ-œpc•@'¡ùxƒ@—1@"ÅŸ?ïþßF]C¿èÏÊ÷›¾ž¿çHìÏ¿é/ّ×-yUNASNone?££³æÜI?¤«(–¯ÖÞ?Ֆ ¥³?Ï¿`»à?äv4˜@²?Ï­‰W?Ëloٛ?ÐË´êz?ÆwMÌ3O?¿Y{⊵?ã¡püӌ?ÏÙyb?źw*É?­g×K¤ñ?Í+ÉÌ++?³y`G¡%ë?ãFoÂts?µ¤þGÉ6M?¿×€ÍùPA?²H'-í\?Á'i©W?´çŠXØ
?砉p»C?»¡í2qž?£b°P¹D?§¢<§ƒR?Ô$'ö+/?Ïn3
)µÂ?ä¼Â±ž{´?Ïwº´2?Øe=JÒûÕ?ӂ•}€+?Æx†Ïg†Í?¿ïْê7?Ü^Lf`?ÐAˆ
¥öI?Ñ×´ Gb?²=í"Š?Éç"ä[‰¿?¯ÂDÝ¥n+?áËlØùß?µ5úÉ•Ì?Æö.…y|?´z±Ů?Ȏ]VÙfÊ?²xãûïM?äÝëGG?º›ö€i6OTHER3FGL J1813.6-6845@tY+jçÕgÀ5ؖÝ&·$À:0ÅJ!ŒÀ;¸¨Uôÿ?ë@…ñh"ñ@…ÖVÍÂ@9þgú?º'¡0Dt¿ãn¤ç?ó¿íDTd ¿ßHQŸÒ:UNASNone?íéÑø°«Y?²†ê^à?¢¼ÇN¼.M?©†i(G#?L2SQp<?¥1î÷…bI?í£Zº®´?¼Å€EhG›?˜VRÇøý'?¦In»¢í{?©Ÿ*ô''ý?¶95š…k©?ë'ùý§i?¨'¡~(?³,îáa¾¾?¡(æ•U$:?°;H¥Õý?¯_S¢"?èɳÛ9L'?·Ü('§¥ü?¹Vj+(3?´j³šO5Ã?À-û}†µß?°¡gi©A?îÍÙSº?·'²Ëx?"g˜Œö•k?£sûö1?šÞ¬W¾+??°]Ά±©?ï;ÁepP?£ Åèïý…?€!OÊއ?‹ßŠÕá'd?w5¬åDÌ?Ê#z-˜•?î¼ïMïç?™L±)EX+?¡Ñ™QŒn?'Ë$`oq÷?›…/q‹N?GÂ?î%~×"?œV:¬ö®ù? êþ^8q?'~/÷7±'?GB€xÎ?ÙX«¥¦;AGN3FGL J1813.6+2820@K¡rGE8ï@4,ÙÆ°SÀ:0"t¼jÀ;¯M†›¿¬vä"`@
EiÁƒ@§†€b;	¿äj4Z`ÚÇ¿è=&ÃpX¿Ù± ˆ¿ã%ü¬,'UNASNone?ïÒaô²"?uVrÉeU?='S¿l/:?:Ҙ	õ?týÀF?t‹ÜÏD½q?ïZ…`ìBÎ?™Š"+™£å?²ÌÉÜR]?€Èöâ©Ú?‰…Afà[`?•îºËQÿ?îz'0WœÛ?›¥xÐc?ŒíÜPž4%?wðqF.,¢?¡e傾E?Š%ÁÆý?íù¶R•»?•²ÈÎÒø?z[Oè躩?u¡ªûÚˆ?­0Ö÷?"+§ÞKN?ïõVe(?t_Òrý?)Nn'UŒ
?(¦5ù¹?Rυ}D±°?tE㉆·Ï?ïÉn´q>å?|!™d3ëô?eԞ,BT—?a!îù·'?p^Vº._?vØÕ¥?ïlþÛ螏?vþ|✟`?zŠŽì›äí?cƒá6Àù?‡{ž¨±–?qæ/€}œ?ï€Û½U‹x?sçòŠ§?nH¹ï…Í?W粺¨Œ?ˆD¾mZî°?qVÃ%ò‡AGN3FGL J1814.0-1757c@)ƒÅ›€#§¿Æþ§°³'À80RÆvÀ9ŸY—K
À?íð}ø9žC@NÎLBy@s&@©?ïþ€ªú¿ã+…Æ9F¿â—y';|-¿íb=/òr4UNASNone ?n?:aª†Ó?lÜ¥4
íä?ɍ4™Ã=µ?ÇúÙá™sÀ?é~sŸH<?È!Û»ÖÝ?'òmßñ0ž? ñ*feL¦?ÇYU¹´±?½[C{2ƒé?éš+»ÖÁ~?À;‰c@—?¸R§Ñï
?¤÷™8§?ÕÂH­Ì?²›©o¶­b?âfÞJÅîY?³¸bôD2?¨cý!ö—C?©oגôDþ?´Auéï¥ó?«©îMìk$?ëñ'pçYý?¶óáQ:ƀ?aßÀ€Ggå?gøµãñr?Ç^äuñ?È#oé?êg=¯kœ?È&%½˜–(?¢;'µ÷4?³GS(U?ÐW¸£3Ý?¿J쯸Œ?æ³ðDÌÞ?Ãof;U?Á®·
ô?§0¹ŒLUÎ?Ó}Sð9…Õ?°æIIWßP?áÕ¨Dœ?²—˜R:Ã?¨´ÃL¸˜Í?°xmîY?µÿý™ÑÖU?¤b4Iҕ?ë´´15h?µÜ•Q<[òOTHER3FGL J1814.1-1734c@*5¤i×4/¿˜¡©¢?hÀ79™J¿@óÀ9tõɯâ?î:ÕG*ó@*bÐYÊ!@_R`u
Ä¿äüoÞùäͿ菪î^J—¿éÔnÆ $¿éK;eé#UNASNone`?wÞ[cR³ ?xˆ´s÷^?·à`£9óš?¿àësQd?ìÔ74þ%?ÀEOP±Y?šò'‹Î?£îä—ÍDJ?Äbþ§æ8"?»Òzm¦Ãñ?êÁ£?¿µ 	,F?¸«VÔyÊ?¢4ÉÀüÏ?щµmWÙ?µ­N÷ò°Û?ä:ïÞ'p»?·{÷ÒqíÒ?§pNOKö?§ØÚÒçù?¯Î_©EÐ?¡í"ôl˜?일;óÃ?²E$߶Èú?iš{†©û?nÓÖ")TF?¸™BÿÖzÑ?Á
š1]ßÉ?ìÓ=$GF?Á5V<çUÔ?©C™«î?µU'#´¥?ɏĔÖ!›?¿·sšèŠT?èÕ@'§(?Äѵ{ÄV?¼ˆ«0
m?¦ôóµÙf?ÒwEæWý?´Ämýs?ã3G¦ÃßÏ?µ¿|^¸:?¨³y`0oÉ?°BâìˆyÃ?¯F®å+"?™Ü¢‡ó·š?ì€]{ŽÊ;?´cÆàåã"OTHER3FGL J1815.1+5919@VÛ"Ðå`@; ¢G'ÝÀ:þ—J4À;Ñ-åìXƒ?î6,óå@ÃQžƒ8Y@‡ÿž[J¿å¾rMi.¿éWȄÏÄ4¿êTq£J6I¿ïý›¢ÄvÎUNASNone?îû tK£º?ž´ú¥÷?«O#©¨Z?ÜX8®ÐÁ?¶IéÞ'?•T¨ÅãM?ã퉨,Q?Ņí8ìÊ]?ÓàߐHã?Ã	·a´-¢?·À<6£;j?·¥Ê0щ>?ë
0œ™Âù?ªT5|Ý£?¶RÛªlAö?¡ƒ|Öþš?±[ŸpŦB?›ëL[ü"¶?Þ*j¹Ô™í?¶æûìÝÔÖ?ÜF¨Íál9?¸2w7!³?¶;±ä)å?§3?f€D?ïO>²ÿWu?"Í>ãAc?‰Ëp)©^Ã?‰Þg•?¶²?'dã#7Qû?‹°9Ü)=?êtá¢XQ?¸W«¥,AI?Ào©ëFß?´º›¢ii)?¦ó>-e¨v?¦ÓpñRë?í£‡õéaê?š~«½Ä­U?§H­™°ß"?'¨©øyˆ^?œý¦
J™?ˆ ˆ¹¸Î?è똵¡•š?§mm‰à?Èç–ÎI_×?¤WªIÚK?›P2ÔZä?þ¦T69ØAGN3FGL J1816.0-6407@t¥e¶™…À4"ÕA"ÈÀ9r"#—µÀ;¤mµ@æ?æféšõ@~6QJËU@UŽ >¹Ï¿ã©WD_€n¿æX\ãZØ¿¿æÏÜ°´W$¿ïÿ:g|]kUNASNone?î'øàü?§¾k` Q.? V·wʾ?¤ ÇWºHˆ?Š&ú¡¹|"?‹lv&Ì?Ý`… W<Â?Æ®6 oÙy?ÔËgŒu³?Ãd-åI#?˨&¶^\"?ÀõJï^ê?ë¹¢3N¿‰?§"¹"?´_ɨÐÐ/? ýp>K?«¦Iyrg?"yÑfà@?à‡c)×%'?¶Ë(HQ?ÓÈsTix?¶Oƒ6ÈíY?ÆQŒ±öÿô?®Q'…?àÏ@Î?É±¡Ö¹?"î¯_N{*?œšeí%Ï÷?q԰ײެ?q5-¼ÚD?çÍ1Ë÷\:?¿¦v!"?ÃR³e6]?´¶ÓqÉ)?ºñ
ÕØw?²Ù›h+—?î1þ,–6
?"—(Ý6Ô?¢œj'ùÌ?°
Äü®C?"‡eL{|Ð?SÀ™*?êÈžÑù?¤Fë‹ð?¿Yiþ¡[/? qߥÉQ?°(UðE¤"?˜ºf€®	jAGN3FGL J1816.2-2726@ŒS£C^À€`îWaÀ9Û6òÛÀ:òyùK?ÀõßÐyn@ý¾ž
ío@aHu«ÿ¿çv¶ÑÉó¿æÙ;®_ù¿Þ™±¾Jö¿íLøÿZ¾'UNASNone?ä9›±ïQ?Ç/NƦ[ä?¾©R1P/?·˜Ök« Š?ÏÅ
!'?ŪØ)æó?á1˜ÅÍîÐ?͆ˍÔá¼?¼øZ¼†zû?±ÇA±Eõ½?Ö^·ÅBƒ¢?ÉEŒÅ(qA?݅U2,æ?¾÷Âp!ü?ÅäcŸë ?¬=¦EýÐ?×÷¸.¾H?¿\jŸ*?✝M5ñ\?¶õÚkZ?©¹æ
€¾?šn+¡"?׏ˆ£ýö?¶w_ÅeäÜ?éã˜@S,?Ááo(#W?²ý6‹Ž†?±ˆlHô(?Â֔ÝÙK?¼zÏ>—"?é¬×⳩?ÂO ²?­‹ÕG·?¦¢ ·Ãk?ÁéÙÁ +?»Û¦nê?æ²c*°?³­þÆ
"Ð?½£û·	Ü?¤'SPëó?Æn¡í¿ÐT?°-ñÖ¡«Å?é	‰Š€U?¨$à—×c?¢¿}§êx?ŠÒ^&éÞ1?Ç*ñ?¥ûuu°­ÉAGN3FGL J1816.5-1145@2}	¾º@ŽœæU4À8x‰žyÓ+À9ùÛån"B¿ðfÅê/‰0@8Lø1@Øbà¿ã¨ÝF‰¿ç¿©ò	ûµ¿émwâß¿âaÚK̘[UNASNone	?Äým/¥
?ƒ±Æ<Ÿ?²{ñ0¤û‡?µ*ȨZ	?èq&Ž45½?ǝË*z?ß:²!¿‡.?Õ4©pãS2?¤Ðä™ÔK?£oÝßÅ?Þ+1JêxÉ?Ô-â÷[–ª?Íݚ–TüÃ?°öî	bž>?Å_™©Åó?±í¿:Ü؅?ãCt‰¿²?¸;}—¾?ÚNµ£C8?É¢j°okj?bÙΜ<'ƒ?båUóe1š?âÅË_J¤z?É¥"ì/àæ?¿Z-Èæ
f?¼€x9¼S?¹xêFú:?¾!G"~Z#?èåœþd/¼?ÆOˆå~?䌣M2Éè?Ԅñ>ò?£ùÛÀPŠ?¤9$Y"©œ?Ôg~xñÀ?ÒÚ8w"‹?Òn*Öÿfä?±.•X$L?ÆV×R6Ú?°wy\W?áHß5/7?µ>ÛbÌ2?à4âS'ð?Äü|?
(?UæÇG§\?M‹f•[\?߀UO蠓?ÄùêKQ¦ÖMIXED3FGL J1817.3-3033?ÿÙÞ7X\À+àÞ҈ÎÀ9ÍâÀTÀ;+	¾º?½Åƒö;±@'mÖÈ#E@v?@\¼o¿ãª"
õZ¿èStM9ſ冕l¿ããPM[Ž­UNASNone?ïT0#?œÃ['¦?`
!{¥½¿?_jÒ(ýµX?šSˆ"ï?œ4;c0æx?í)í"
†?¹qÊeå?Ž»«­¼h?–"‡š°ÉK?²ÙébL?¶҆ ¸?í±+.ŠŠ'?ž¨¢G*?–Õý€Q}?†"N]úê¿?©'Ás7?˜x–i¹W$?ëeWõ#Fñ?©EÌ)hË?z•]ùÉÖ?sµdÔ¥
?Á•õ;<'_?¨¢ÁRÊ?ïÁšÃÔðL?"䈩|þ"?I›í •r?GÖUŠˆ?{ÿ yúA?"§'¡že?ï¯\' ?¡‡9ä‹?veqÖ%uä?wz›Ž#·E?—p·ú·ÿ|?¤ã¼·Ý¦?ïEó¨ï?ƒðòf§cc?näº?pªÛǾ~?ùì}‡¹?€Zž«î?î}®¸JðÐ?Šaß÷†?r%ÄÉ<Ü?]"ºmY_?¥âoé¯ß?ˆ—qñëÝbAGN3FGL J1817.7+2530@Jh'¾‹Áj@2Ma€M˜9À9ï6¥®zÒÀ;Œo[Ømë?èä¥c§DR@•·+о@¶Ÿ¤n¿Ý3X$·Íë¿êù^QÊ¿âoµÅý®J¿ïÿµš1DUNASNone?ïÛN#"FÞ?mî8¥ò¶?XƒoÅ?U¤	δ,?hp%ìkk?h"0
}XÔ?ê¡(Ï,#?»0J (È?¹ß·ÏÔWõ?°3'‹ï½?±6猅y?³
6üËf?ìúö"š§? Yx+ǂ?¨%¡]ý?"܆så"?§Ãq"dÖZ?"p¼fßCX?åM?CÀQÈ?µ>q"(µ0?ƈd•"]ð?²ýºŸÉjŠ?ÄBž[ÜZð?©¾Øçd#?ïòçàñ¿B?X!:^1L?Cƒ
´_F?FCpŸë?Pn·tŸ.ò?PXb'ÕB?îŒñPËÜ?¥+nµî£‡?¢'Vs?"KLq­X?š©A.'îw?ŸNßÈ8O?î"?¥\pn?Že¾ÐÔ§?›T!è~?…ïCä7?'#é»±K±?=&š¨Ë?ë;ÌN͘z?ž7¦LLO?ºGzR'!?™l€º"ß?§´FoÛB!??RAGN3FGL J1818.5+1320@D§¨ÖM@*|õn¬†À:&ÕÖ`ÊEÀ;Œ¥ÉRÄÉ?ëòm–¾@æÚâå@Š`@²x¿éžˆ‹v¸¿¸×mÌ ª¿â¬"ÀcT¿è'¹ø‰¿UNASNone?ïWpÝÁD? [hLÕ?]µlý½?'"²Ž[n?Ž÷hSfß|?–#¬«ºÆt?çm²'ô'?Èí]†Bú¦?Â.ŠÄx?¼!š]Ӊ™?Àÿ%˧Å?Àhõwb?ìܾYÂi?£\šëÁ>*?§³Î6úÖ?˜+?¯ÿrÎ?ª€L1*<?—5FG‡ßû?⹚³uò?·ÙØ¿mjq?Òݨź?¸!Ø s0,?ÁÙà X?©þÂKì?ï¶+çB"?'ïÒÑX)?rïI싘 ?uA­-üæ¼?r f:¸?v|åšØ?¾?í<˜¾Ra?·IÅ©&†P?¥gçmRŒì?¦%í·ihm?¦ÖÏ4˜
?®	¶_"‡ˆ?îÄP­J.*?'PøþÊnû?"ÿö`h!\?†ÛB@Îî?"uóïrák?'W8ú\!ö?é'ü±ªÌ?¥53|Nó?Äø§/?£²
A¶ÿg?©›Øt\?õ)CbƒÂAGN3FGL J1819.5-2045c@%ˊ~s£fÀ"Í*1,À8÷þ×0À:‡Û…Í3ûÀeVWz?@qÛøòÆ@¥"úI¿ço-5B¿êåCÔɤ¿àLyõܲë¿æVÈ¥1
¥UNASNone(?ßvN»ÏÏ?Ìîk¾"?{`À·Ñ:?{å†~H(7?à>ƒVó=
?Íg{ pŠ?ê拔*Ê?ђìä؍?‹âx¹,åo?¡CUØ39<?§ª$<†?нPÀ.PB?Ü~dŽ8×&?º5¢¾ë?·''»[¶4?¢(kó³?Ý·ºÂð;M?ºN	Éé~Å?íj	<Oø¢?¶¥ßŽu˜>ïÚqˆ)?ٙ"þ7?´®·J­?¶~BµŽ?æ"B£V%?Ìç «º6%?vøŽæÇþ'?yÜËé¿?Ò}˜}v¬?ÌâÙï8÷?ím€žËݏ?Èz‡O\?"Ê0Nk?šeA'"4ú?²Ã¿%þ?Æ|sª,ö?èDÁÀT?´˜±{ÞT?«&4Ôe?™Ï…2@?É5&TŸáÕ?±ãs}?îî‹
E6?¡—³·î>»9Õ0j>Å>áÍwx8s?¡·'9>?¡—›G¶MIXED3FGL J1819.5-1345@1mÁ¤zž?ä©À°ñÀ7éÞ(>ãkÀ9Ù)Š=D¿óÐý8zoÞ@jÔÙ`®ì@Ò$ ›«î¿ãŸ"›
jª¿ëCS‡ªó¿äêžB²¿é«F{©3UNASNone	?¡Šµ¥û?©ðž×â?t"•Ÿ±Ñ?ƒó,¨?§È?ðSÔ?«
QNC?Ôã|ÜÊpÒ?Õ‹ÊŠ8?¤÷hhàn^?£â²ùME?ä>Ë!?ԗ[;eé?ÅÍ|egt?¬ï?*Åù?Ž—áĽ?°úÙd/¶?åG:dĕ?µT.L
óä?Þn"†Ñ°?ÊwÉÝ{"?Rç·‹?UŸØûÛã?àçÕ.p*à?Êסo¯n?­;$dÖqÑ?´¯BÒêF{?"RDÞeØJ?¦øyk)Xd?퉻'è¥p?ºj>ž\ˆ'?ÛºÃÔD?ØHE±•?ª"Nâ\…?¦ûí×Ìi¬?ày»¯æYˆ?֛«Å|?ÉnwNb†?®ÉðÄ5¿ú?ÇÓ	-asI?¯¨b7Â3ù?ã«bÔ
Œ?´…'ØˍÑ?ᴂŽòˆ?Ē¶ÞEg‹?F±˜²t¢?GV3Dqˆt?܋øꕓ-?ĒE'[aÐMIXED3FGL J1820.3-1529c@/Nñw§Š¿Õê'nQí3À8>ö%‹ªÄÀ9z«Yµ}ü¿ý%1¸^Ö¥@uÌKȀb@¥5À9ü¿èˆÑ§ÊVG¿é-XQ¿âA¥WÏ¿ìH	èrUïUNASNone0?'á‡m<Üd?šçÌóÝ3­?­4å×î?·Ë¦øø†?흪æ*Þ?¼G¦:op?à·1"?x™?×yVÖAì?¥*Û§¯Qª?­˜¡Ø–†?ÛìBFT*Ø?Ök¡™mNã?ÄÙH+ùê#?©ÿך"ç?υáûKÿø?°ko%+ým?âè5v.…y?²éfïÁ½?ÍÉ3Zuli?͕ÖzW?M¢ƒ—¤è??Vü³ýðq?è†Jˆu–?Í¢¸¥2³?|ɼé0õ?‰â 'öM?µ§7wF¥¯?ÁÐdíüƒ…?í…—ÓP?Âiß­$:ó?ä†x6Ñ?×ö½áø?¥¢º³"_?§Ý'ç9Z?ÔS"·²‰U?Õ*€çÆù#?ʖP'ÐÝ?¬|Ì&±0?ε,òý8?®ù¬buËF?áÓ>´yL{?±ü§X
?ɒoZùP?Êc¦ CJ
?:?Qêš?F'dŸXQƒ?é˜>؋z?ÊgTÂ\ÿMIXED3FGL J1820.4-3217?ç•3­ÁÀ TMryšÀ9^ê䭔À;2;Yrb?ó/ÂÖ(ì@«©Ô¥3V@À]€c½•¿Ü]©¡³Í¿ã˒ìgƒ¿æ·°ÌC¿ïÿfh¥ìõUNASNone?Ån"í)¨?¿sDÊy$H?áÈ@Z'»?ɍƒàö?Ѹ5J(†÷?ÄNj`Wô?¹Íƒ
œÏ?¹"¹g?àq"í¸U?ÃH~¸±{§?Ùk¼â¨#?ÄHòÒoú?×çø;)e™?´ôÜ6¿]7?ÜGœÕ%È?µ[®9K¼?Ç ×fé>?ªÍËAµÂ?Î DŠà›?©ˆ¢­<Ú>?àl0PÞG?´³š¬i*?ЯZ\S#?¬÷ôKt{0?×°™À°ß±?È-g»¿Íû?ÝL‹§¹?ȵY¦íó—?ƶBœ²©?ºíÂ%ë'?ΈՎoø?Ľ??tÎÎ?Ý{µ´hŽ?À|N€Ò´?Ó@BàÐ9ê?À«	õ]uã?ådX%Ÿ»‹?±´üvˆ?Δåw5
?¬éú`'ã?·³såsðd?Š($›Çš?ÚßàáèÎò?¨ÍîvsW?ÛïFnú3¸?­ß²QÚ?Âa±^9ú«?G8H§ÖÍMIXED3FGL J1821.6-1436c@0'j¨ëF5¿É'îz°À7ÕõŒ·_À9±Ããïÿ?ì‡õÁþ)@í{µƒ@S<À¥¢?ïõŠZCÝ¿âU¤Ÿ‡d¿âý5ò°P¿ä_æãUNASNone ?Æ•"ëù¨?'ùáJnt?ÁAn_Y,?ÂÛ_øúí?ë9º÷ÀÉè?Ãô«Tb?žìË«ö¤ž?¦h›ÁYTš?Áj'Ó@s'?¾tx‰î?ê­õ.æA?Á4#‰?±\óöÝA?žþu)tI?¼ª«(§?¨Pòõ"è?êQŒ+¿Bî?­`¾XV3?ªŸ¦9jN?§¥Ç&ÿúö?¬[éê!Ãà?£'SÃ%Î?ì˜×fÑÍ?²
•"^?ÍÑKåñ1?—%ái{"'?ÀÔÅ)?iw?ÃÜPq¡$?ëK—pÓ}?ÅJôƒR¸è?±edß?Ñ?¸'M3µE9?ƦñєÞ?ÀoÔ|^?è)¢ÿQŒî?Åíã2iߘ?·Œ?DÁÅ?£"¹ÛÕêˆ?¿Š²‡7~?§}þHõ?é,Áe:—?®U)ƒP?¯Fj6nk?°ÀŽx×;?­G,·´…Û?œºhìÅ¿?ì;8Íü͛?´õ
£aOTHER3FGL J1821.9+6636@X"LƒfQn@;£ŒSâÖÀ:rˆšmÔðÀ<Iqc?äEO¶²ÀB@ð`™ËX@S—Á¼M¿ëóL´ÓK¿ßuÖ¤o"¿Ûô¹"'¢¿Û
`ߌUNASNone?ïöìqL?E;åFÖøD?AÏË9õ"?<-i¿U"?B€%Y»'?6îž)3?îÎzs°ô!?¨2›ñ~++?""õ'x¯?©¤ÞÚ?'œ'™ám7?žÁñÙ=…?ïWæ×÷	?o"‡*?"²ƒ¥r©?r—‰1-?'»Á'Ï-¢?xÙ,èOŽû?큽õ™t±?¦é­_øwÆ?¢fdSŠÃ?¢Ö#½¾IÏ?¥àº?u6?—eeVé==?ïû'ÏäÀ?4ć'¸]?/c
Ú·îb?&8[-}¬?7²ek£°A?*Q»V©?4?ï®â·MgE?†kmª?s¦ ô•á?v¬'ò'—?tþþ+ù/è?ÇXËqx«?úI?qìxցߚ?xòà­3eA?h!ÄýžÇn?'!¯™µo?f#mu¾¹?ï>VxcÔ?‰´.0c?Ï||Ð0?"°¡Òò?}–Ò!I?spm9€AGN3FGL J1823.2-4722@u°í(ŒçÀ.R‡;©À:И3hÀ;ŸÁ}ä1m?ô)Óݍ9@¬4VHáñ@TÿÀ,³?毐c1u¿Ìŀlßk¿áq™ô™€«¿ïÿô›.*qUNASNone?ÙǘÒÁ¥Ê?Ò½B֔KÒ?Ùc}'P?ÒJ‹aC‰?ÊDaQJ?ÈoúíO,?¥9ñ
/À?²Û±ºIRß?é7è¸vå¡?Âd‰
ý'?ÅÑà»t¾L?¿ãáøiCø?Ðûqù ?³Yv½c~?áU~†1¡§?¹tíºCg?ȳ!óù?$?²D
°²?Âv¤Ìþv?®G†43¤¢?è,
­›?¸Ÿ"ÃÄþ\?»ÃUø–:?« ÅšÄàò?à›n§Â@?Ö1'ŒH¼÷?Òýuӓ)?Ò±ÍVŠ?Ǘ[Yuš¿?ÊÑ~É&®?¹¤•ÿŽÉ?¿iªNÙ¾?ç±¼ÔÃL'?ğ"äMòÒ?ÄfÁ«§µ?ºç`6v‰Ÿ?Þ&!'9³?³¹ä?Ùæézú¿?²s'è?Á‡ïr%ž?©&~HÒ?Õhò1á$?¯Sl±Ö'£?ã$¨ð	ùå?²ÄF%E?²u³Î?ŸHýŠzMIXED3FGL J1824.2-5427@uE	k¹Œ~À2
cÇOµÀ:WL0À;¯rçԐ?éƸ	µû@}ò

@¥ØߪŸü¿ãYÝUtëS?®ì:•ñý¿å8S¦ù²¿í"vmUNASNone?ì݄k›?È?±G×û—?´ªˆ(}ْ?±øæÇ ?'¥QèèÒ¶?'BpB&N?áœðíy¦Æ?È4ÛIA=?Ð~W	Xª?Á+´An<ý?ȏŽ6þ³"?À¦=C#ã?ç0…ŽŸÀz?±c8Cõ?‹?É	" `T¡?­Inbor?´iŽH‰"ï? ¦]óâK ?á°U©î¶?µòèb¦ÿŽ?×ÌZT?¶ÒžäUVS?¶û"Àû{?¤qû‹2@?í·»jq/e?«ãw&Z»@?®¥m?ªØa'¦—??‡|Å$A:Î?ƒñ*¼wƒ/?éèm3#Ú?½Pµ=þ­?ºü$ÔÒX?°æ«ÍÒ?µÀq"£Ý×?±«ÂêÍs#?êŠÛ#3¿?¨½žÈŽ—?À{ôÁ?¥AÓÀ"1?¥e÷Ѝté?"[JýŸë}?ê_ÿÓp'?¢±hÀ¤C˜?Â5ªš%Ž8?¡BšÎ/Êß?¡)Xeˆ=?Ž‹†!ñÅAGN3FGL J1824.3-0620@82Ø]ú‡@©U´g{9À8‹'®›‰^À:š'Bdÿ^¿õù}d¯­@
éGZÝq5@òø‹áu¿ë(¡–­¿áҝç˜;¿ÊwÃÛâi¿ìè2a"³UNASNone?×\$]ñš?È×ÄÍyñ?Ý"כ\è8?ÉÅ·[îµ¢?Ç"ŠL[?Ÿ ­Ï?æžíöh?ÑsWO…?¢©d½ÄÇ?¦	–?Ðl÷|EBL?ÐÈ£PX?×
¬/7>õ?´øyÚ#?зàÃ
?°V†´?Ø:s«Î¿?µ"xÌ´<ø?åº
V´ÜZ?Ä­ýkƒº?sfáÅ//?€Ã:ù5l?Ô?é·5®/?Ä»0î	ˆj?à]³ôÜë?ʉȺ³3?×Wzdž?Ȃ¿ÅIÃ?¿µîpØҌ?½éõ?ìGf_Î?Ç´4Q¸¦Ç?"=Ù?œ™ë§ÿÖ?¸á€ŽrÙm?Äã
I\5?âåd^àqV?³á×+¥"1?Ȗ»³9?«#'pÿgA?ËÔ]sèHî?® H«Ý—_?éücñʐ»?·ä>
ÄÉ$?_bº`ÑL?b‹Ô«±¨¾?ÇϪÂá¼s?·Ó_]¢%MIXED3FGL J1827.6-0846@6k"Àh¡?óݑ[¶ÓÀ868À:;¾íæù?֘nyé@I—M¹ò@åÎ 3ý¿çAT惤‡¿ã²')Þu¿å·x®¬?'¿ççÁH›`UNASNone?Ÿ¿%~ƂÑ?¡r`O?±º³^€'¶?´7D"r›?ìÊ°hpµR?¸Й(d?ÍbŠwqN?ÊU[³ý?~?»‰õ]uã?³Ó<½‰5?å6¶Š§J?ÊtÂ{ mð?É~Í>?°:!­Ýoô?ËA#ªvƒ?³Ç¾Dù¨?â욃,"{?·ÓwX.É?ÍÙ%˜s"?½ÓŒÚnuÿ?©¶PŸÚÅA?•¯%qÿvÃ?æîQÈ=$?¿hdåª6?±É§
gÚQ?´ÃÔû}?«ÈŽ1ƒ-?²	'_oz'?ì
B;cÙC?¼úJžß©ž?ßfõ&'?Ò
Òæí4?¸g)–­t?²%Àw¥>?ڀ!ü‡®?Ïÿ©õBð?Ó}…l;¤?´@Ò
Ù{j?Èf«GccI?°ŠçÅK¤?à''x	ž\?µÆÃع=o?Õ/÷òóۍ?¿äãY%¯?§/ןhÚ?Œ']4 ?ã÷áÕ!ì?¿ÓÎ|WòäMIXED3FGL J1827.7+1141@Dd	þ†ƒ<@%	Ž«ÿÎÀ9›iK4ÄÀ;[ C×Æ%?õe3€µòì@
9r&@år?ãoÑ?î4~{ŸÍT¿áp$2íÆ ¿áOþðáT¿ïÿð	V¯©UNASNone?¢0×]Pfk?°½kv׳í?âŽ#"F*?Ó.³Á&ë?؝žênüÁ?Ón·%>m?.øÄÿÈ?¨6–-î³?é³Z@ñÀ?úgÿ\†?ō£Ä?ÁÕë!p?Èó' "?®±p®qu—?äw¸!³È´?¶î¬‰›?Æ+èJ%?®soçè©?¸tÒE҅?§™išŽ¼:?ç5÷ÍpP?¼ïõP$?Ő¾ÿ"¯þ?µá"…?©õHÔ˘?·H{·ÿÔ?ãCë3¸?Ó=äàry£?Ö²Nμˆ~?ÓLV+{?±û¦×@½?³¨¯C÷g?裮D$Ñ?ÀºÆ‰»;?Ästty­?½80¼®?ÚdNÅF,?²X<La'|?Ýu
6?³æÛL߅?ÁÔM6ay?§7£"Ëþ?̇fmë?¬¿õ?å.+.ó‹?´êUW	!?¾S˜#‡Ö?§¦Ûi¦?xPSR3FGL J1829.2+3229@NRs×Ûõ@2"Ø#B$hÀ9þJÁÅ1ÎÀ;¯Ux™]?ô)ÎØÀ ï@•kâ@H?ìT'?†F¦¿Ýl0%Ú'¿çÈRoò¿ïÿÆ:Gµ²UNASNone?֍B•ž/?ÉWôH»0?älzíºŒ?Ê1$‰»ïÊ?'C||^g˜?"Pþu÷ç?Ì«þԏlx?ÁbzYɆ?ä;•¾Ó?ÅÚ;O?Âgæ×m˜<?Àà¤× Ÿ?Öõ"íQ@?¹küʸÃ?à–uʖ?º•ÂßäÆ?¿v åö?§A
éÓ?Î,ηªô?°4'Qt)?åÔ}bC¨?´åêôuËC?µÿÈZsÕ?£¹ŠëIó;?ÝÜñý!Ã
?̐8¯°C?à¤òÉiH¢?Ìä-bç‰?‹%
÷&¢?v¶ue?ÞãOa"jõ?ÃNÙ³KW¨?Ú,sY'Â?Âäo‰Xa?»Â€®I#?¶n4
"6Z?ã5–D?³Ó&Y`8?ÔÈp#K&?²
Äï9²t?³1TR?È›&ñã0?á&A÷àæ?«
 È$+?Û6" >ö?«f.Ü:?¦çD]î?"vςÒMIXED3FGL J1829.2+2731@Kæe+ÓÃ@0­Å÷Æu›À9lg"cϳÀ;Š¦Bˆ?ðÊÅ~#òN@'‡µÁms@õЀ5šl¿ãÇa/Åæ¿êbà[09¿è'íþÔ:¿ïýó®Á|•UNASNone?í9w½HB?´¾åC~>{?­¤'•S±?«R¥b|V?¡Öìxs5?©þq´ž
å?âµûÏï—?Ä`h¯…­î?Ó%Üf%w?½õ»zâA?ÁEoDu>µ?¾¯U;#u?èÒ›X>?²j".dR¡?…ôê*ß/?«ðg²pôí?´c…õ±²?Ÿ®–(—2?Þ]þÌ+ð§?±§ìy­™j?ؾ¤L¦?²Øþ{0ýî?ÁÆè@_…e?«ŒÝ0µŒ?î6bvö4?®ÅþJŸë«?¦"<Ç"í?¦tÚ)?Š>V|äW-?£1͵-ˆt?薲¦AÉ?»Kl³\Ž?ÄuŠ¨‡j?²ü
s[S?²_ZlRљ?±x¨MàŠ?ì¢py©~?¢üo×È6?²D×?To<?œê#"ErÇ?¡OIç›(g?Žn~Q®bB?çàv>dƒ|?£]Edêå?ÊcH­š?¡=ÍE?¨k{ÏßD×?•ÍÓÝã AGN3FGL J1829.2-1504@1ÉêpLÀ`QyoW§À9$¤úö¬À:ºÊ9t•Ô?íE!@R¼¢@PԃÐZ?ù±Iß/¶¿ï\ ރ׿Ç2"J¹¿Þ†$æÙR¿Ì­ÞJÄUNASNone?çÏø?00?Ä\œKƒ>Â?¯s¾#ø¾Ô?©Ûí³j'?ËÛЖ‰?ÃjÃÕRO?ÖIŒ¥Y/5?ÒψvåO?´Ô×Ñ?)?²Å"ãóÙ?â@žÌfþð?Ñõ‰ôû?ãÙº¨KÒÖ?µ|ˆäW½?ºÙ·j1o?¤4_3:kÁ?і&€zí:?³vûAcÔd?âÞ%uì|?ÆI"ž:"$?£%r¢¬4H?¨-ð÷Kû?Ù}•`¾ ~?Æ:ãý¯²?èóëîÑ?Å¢žÈO?¦N»³v™Í?§×å%'¾?Ê"¢Í±
?ÂoúluÓ?ã#œÜçn†?Ô,û½P-?®z¾pÀ;Ø?¬Qò¯î_?Õénxم˜?ÒŠNŠã?ê-×Gn?«Õ¢"ŸÌ?­Cç§?˜ÿmŒaî?À7ÜT?§èŸÕ§ñ?æÆnÇ=t?ºùü§Â
?«)qŽCÂ?¢éê&ëJ?Î ý•[`=?¹õxÆcMIXED3FGL J1829.3-0135c@<ýæ>Ž@ÀgHäu`À8É2=jÀ:hƒwe?áŸ4eã3Á@
¨×z$ß@JMà]£I¿Ñ-ðŽHÌ¿ä¹ï[ ˜¿ãWìEÒ·¿æ¿ÿL¯c¹UNASNone4?†¦/‡µŸ?Œiâùˆ7_?Ÿ é!ʳ¡?£EüB~?î¨_ùŒ?¦äïœD>ª?è讦WS_?ÍÂÉ[ܨ@?©æq•¢?±ÿ'-ýz{?ÅãÁŠ=Iü?Ç'·Ža?ÑÐ hD%ä?±Œ'ëHÀ?½:¨mŽ¤?¦ûHä‰ý¦?ãpš¸0;:?³+ œÜñ?Ä^+—»üy?½çè$I¾î?¦!é}ó?š¯,¦¨?é‡BûŽgs?Àj:À_?Ü]£+<?—dnÆ $?—[n‡?¡ûšbéņ?î¾DZEZ?§î>èl<I?ì"Tà¤gu?ÇnlST)½?¢?HäL$¯?²z…¡Æã?²½´‰'˜ý?½ËáÍðþ?ÔX‡ È·ê?±NcZ*^q?ºžÕÉö.?¤Ä
Ò'?âáŒôæ?²'(Þ9"s?ÉøëÓg	"?Àá$-íà)?®yš(h]?"|°§=¡??ç¡mqƒ·?Á"Jûº˜MIXED3FGL J1829.9-0203c@<¥£Â‡è@°ò¿-¨À8~MZü¦À9åÈÂ|ó?è˜è…K?*@©ˆGØ%@åŸ×vI?ì\±àüôL¿áJ~]ö+¿áBö\"(ç¿ìyI{…B±UNASNone ?ƒUâ2P?…¢µg¤€³?æM.Ñà³?Êþ%Ešúÿ?ÒÌÉBØ·?ÊåƖ°c¾?Ö&òªy]0?Ð(Pãê˜?ÓB-:ås?ŵú~ÇíP?ÖÐË(K½]?Ë䏷¯?ÇÊ*'"9P?«=ÃG³‹?Õ²™˜íÍ?²¢Ü;|CM?ÞhÍS°VJ?³‰ðã/N?¤X"ÍQ°a?£µ™\5t§?š²,}?¶ÌOÇþ?êý¦'+?½©ìiJ?x¥÷Òن?"Ûè¡ÿ¨?ãŠER3mZ?ÏÖ|}Bå?؈Ý~ö«?Ïè@Y ý?á;sÚú$?Òz"™û>O?ÌñtטWÐ?ų$ , ?Î »¿ç¿ ?Å(süüëN?Ì8½i`?¬Cp§ŽÎ?ÓyªE¹Gµ?°áÌ|°2?Þi÷–©?²γ·?¨·ÈËä¯?­s{›Ùo/?Às`b?«À]Û?êmfšé¥Ì?·â>£'°MIXED3FGL J1830.7-1630@/Ò¬Ùè>BÀ=Šú`"À87 ޜØéÀ:‡ºÿDï¿ÿ˜!<Ю@"ˑ¹Pn@ƒ>@'|¿éôÉwq•]¿âa¨ÀÂÂ!¿ãèH¿?#4¿è€¾­`‡UNASNone?æ5")S>?ÆêjTæù?³Ö¿°À¸Ô?³$­ )C?Í@?Ê_?Åäó¡Å.•?é‰ñÍ''?Íåśnõ›?œ`¡³÷òH?¦Ç¤7

ù?ÆL'‰9'¶?ËÎ!5¯º?܀/—¿œ/?¸{Æȯde?È,…‹	÷?¯‡ám:7?×i¡­~?µEEFTO?åO@;s7t?ŧáèµ-?oö8V;Ç?~W²ÌJ
Û?Õ!"ð?ůĆà·ï?ìrV@ Ñi?¼3¹½Ùó?œ{'‰0?¡ŠÛŸOEu?µio{A¹?¹T(Ì'
†?í\9ê\³?Áz4Ëë?Œ='ö
«!?˜9Çö?±–‹­҈?¾}ôHM?ç~´¤ÉÙ?´	]ùdÃ?¹¬S^æ"?¤Ê³Ðï7?Å/½hš?­Ùý¸­$?éÅ»;ˆtâ?ºΦì"g?A‡Ý%/¥??P"he,í?È׋4څÑ?¹ÿñý³ÊrAGN3FGL J1830.8-3136@՝CrFÀ#®ç£è`À9·ÙfhÀ;TæØÍ®?ìCÓU–Ï)@
®ññÊ]1@€®_ybB¿ßu¥Ô:X¿¿³ý!£ê¿æ+x±Â…K¿ì8BáòUNASNone?Ä)›†ûÿ?½ÙR=w?櫇ʱ‹ö?Äâ'K]?Á(EN=Л?¹†¦sðÞ<?Óç÷@\«?É—ûÅïÊ?Ö	Ð"í•Å?Á÷
ø{§?Ö8ÃÒ
?Æ7‹3Ç¥?á–"N½?¶xy'iÚ?Ӈír'LQ?³c+XgWú?—›ßçS-?¥ ˜C0Á?ÔUËV³ž†?±†UÞȑ™?ß ®ø{|?·8@«P+?È7ô§Ëû?°WÆhï(?ÐÁ`—?ÄÂ(}"ž?äa–'?ÆøNI¨ÚC?¼œEíb§?´.ÓÍ¥?ãlT­^ûì?Í{`&9^?Èc™¼mó½?»ñ÷1Wï^?ÉëŽ'?—&ð/±?èf¿ëÏÂ?­†Ž¾¸ü¥?Åü4Íº€?¨¤øVð%?°Ñ—~¢¢v?—\ڗ'ÞÈ?ãÛü•'N?©d¿éÊ?Ò^%×F?©l¿{=?½È‹Ów?Ÿ,9!'UMIXED3FGL J1831.7-0157c@<ðÞÁÁÖÐ@źcdÀ8U["¤À9›hýð[GÀ6O†{×@
#nýcÃt@Q¿Š¿ã%ïÓ·ø¿ìxÌwí\¿áœºBÜs‰¿ã–σ$UNASNone0?¾Ðv¼Û?›pUõÍC?c¦bÅ:
ð?t5-,â¢Ô?ï¥^[!†/?žâÖZ‡cv?ë0ßH¥`L?ÍÅGŒwX?‹þŽñù˜?¿wÀ¡?Á|™ûᄷ?Ìʍ¤»-?ËÏ0?°ÕÁ¬^øq?¸ÎC!@V,?¤P(ÌÒÖý?åòvyã5?³ŒÏÔæ?ÓN,å!"Š?άphÝ\?0Õ!$&?4Gò²TÕ?æVÙl²º?ή§R"ÍW?r…b°oc+?'¶§ñƒã?p"¢"9ä?…£«ã]?ï¹Ëõ{0'?™£ò\*,·?ír2ãé/??È3‰=ð•C?ƒçöuôî?–>°ÄøOÚ?±ñjƒ»B?Åõ
'8mÉ?Ñ
7՞x?±
wêQªÞ?»jí+3Ú?¦S'"D?äoA©?³9I¤ÜW?ӚCéõã®?ËקÞÎ#†?$o0±\u
?# Œ£(?æ1—NÅ$?ËØ!T8'lMIXED3FGL J1834.8-0630c@9?î¢	ª¤?ænø`¤Z"À8í^<Ì9À9Øî
5?Ñ𢐟[6@¬fjÃl@²m?ôa¼?ë S0ºÄ¿íö:"`L¿Ô=XRHï¿ÛóÜApUNASNone ?tC£ã
È?û`ì¦rJ?YÔ}WÝú)?lAòñ?ïʎ¥äop?'W9ˆóë0?¹D>sX<W?ĞE›ÃÜ?®sbN-ÿO?¨'ó'mÝ'?êðB¿Öð?Æà5_]]©?ȇúwwR>?¯+e@mû¨?´Óª(xR?¤}"£ÞÙú?çCŒꂦ?²ÛŸdÁ?ĆA/»P?ÁQP
Î8¡?sqw
ÖLB?|®O€"/À?귌ÆnÜ#?ÁšfÆç
H?`ŒF"ÍΞ?tÌ;É*?džŸ.}?†bŽ»P?â?ïÚÕÃ?¥iH¨lD?Ʌn‰ }9?щ5<'š‹?³Ì/ª"äî?¥«K¢º9?ç%hÜôs?Ñb•""å`?Ï?MÃV?¯»uÒäÇ?¶+'ïôt?£sàŒó?åj¼[‡Ý|?±üʏˆÉ?É~Ï9ŸÅ?ÑÓôÖ£ˆ?…ú	*|ÿ{?Lf…ÒÇ?éHd
NOÍ?Ãä†vk OTHER3FGL J1837.3-2403@#±©É'†À<µ]D~µÀ9v"´/GÀ;}}?ÕÏ\t@9muÏ:@6tªL¿çá©	=\¿Ü,Ûàæà¿ãQG¯'[ ¿ï}§SÒ¡3UNASNone?×±©-¾Ý©?ɒ<I²5?àD…cÖ??Ì17!C5?¿00ý×d?¸K*L
?à|hõse?Ís¢çž$?ÈZ+­áWÒ?¼
0·zLš?ÒÚ>)M?Ç$€	?ã:•~?¶ Àl飢?Ð÷¡¸³ ?´+ª–«£h?Á&hsfe?¦k%—-ˆ?Þ× ±.l?¸BHUj{Û?ÈA­Iyƕ?³1±ì¶G?Õª	I?·}½N_Ñ?Þùà'G~«?Ë«_Õ'º.?܇s‹Vω?ËÈÒ)¶S?±ú¯ÊС­?°©"/µ¾?èÂz'–ât?ÆVVÇì?¶"™'ŒiŽ?°ÚUR¬p?Á«É`Ë`«?¾ÑL_k>?è ëÓ«ÁÃ?¯%+¿¾ ?ÄÆFhøš?ª‰Ž-±'T?±lfâN?›G"ˆ'¿?æíwõ"üÔ?­RñP¦é?ºWƃ }? º$*_X?Ç<è#üp?¨]£#qMIXED3FGL J1837.6-0717@8ÝÔÇm{¿Ñ0‡¼øCsÀ8Y­N'DÀ9¹÷[ÐL¿ÐÈlåJ`æ@
Âp¡æð@L¶€… '¿ìpÑVýÆ¿Ìö%°,œÛ¿çÓV˂Žª¿ãËy:{žUNASNone?"2"_ì;â?šûm4õ>?¢ãj$	jO?ª§<œé‹?î05:ۄ\?²D^$¿Ù?»=ÔÝù?ÇÌ>+"²K?´ëF²Ý['?°ÙÿJ¯mð?è³Ç´£Ïí?ÉÁëi½UX?Åó<‡3ª@?®±wÅ¿?Ëхc¯˜?µØ†Ùm?ãŽÏ…R©Š?¸¨—Rï?ËÀB¥Áðü?Ç7=ÙÕHò?Ž
Ò: €?ŠÛ±Kyìy?è—Ä
Ð<?ǵàïeöK?‡ôå,°†G?'Ðqw/š? f]àŽ~;?«mEšX+?î™Æm'S?°©Æ¢96?ЄÅ7¾Cƒ?щÏïcr?·|o@+s‰?«ï›¡å 3?äÎ|
±]?Щuُš?ÊuÂ|['?­™WŽäG?ʉx€*˜ì?²kµ–áj?âÀ1@óBá?µ‡ 7†i?Ë*
?žüZ?Åð•Ÿ"­?ƒÈºå6=?våËajæ—?èæZ‡µìa?Æ?}"†OTHER3FGL J1838.1+3827@PΚ¿3‡@2åxåÄëWÀ9Ù ~(ØÀ;˯é(¿èCc˜D@›@ññP@̾@Bo¿é‡ŸeØÄI¿å;qv¡U¿æ¹˜ÿ"žÏ¿ìÍÈl¸2UNASNone?ïTÿ-ÈN?'ÉâÎ?i?ˆݜÅ÷Z?‡À!àÓÔy?'¡VøÅY'?ƒxì0'?êMë?ª¤&
aË?'Ãu%ÀÈ?"EùFmñ¢?—Çm"yÑ?¤<…5lE?ìÐN#Ïh?¡hR/êØ?©©G4è'?"q¾©átÖ?©ët}Œe?•ýµ֔Ò?툖꒰q?¢t¬xý?—JS t¦?'"¤¦°0ô?«ÑJ¬hי?YA?尿Pzc@?€'àý+Ep?{p¦©H?w°E¼OŒ'?qç,£7Ú?oŒ	$þ?ï¢o
q?€?ƒúŸ8¬ÿ?s‹KµütÝ?tO}'‡C¯?{=.õ6ÿk?†1Ô\Ø8?î3Ñ3
ô_?"·NR—€? ØÄ!¹€m?N[œw´0?—ÔQ\†A7?ˆ?Öq˦/?Ãeñ?{É»t±"ú?h%óÜ:æ?a€ŠnÎRÖ?†QýJYo§?y!oŸË»îAGN3FGL J1838.9-0646@9zTæâ!É¿ÔAKdWmzÀ8:úêíIDÀ9ýèwM>?ÓS–=w7x@RQR-q?þ¿>«Œ`?îÅUÌ)'°?ëL¦*õÏ¿ßÙî7D¿åŠ¯nÍ#UNASNone?Ÿ˜hÏË?žÈA…'÷œ?f(ηP?'ê&l(Ý?îŒû'Aý?¥[ÌoîÍ?´#¾í`?ÄDÒ»?ƌÔL¦d?Á#úƅ5	?çØS
xÄ?Éù¡Îé©õ?ÂٯNjøÐ?«¢Û–!²?­¬5Üéw?šãŠ*E5Û?énа\(Ë?¯«1±"Ù?˹#b/Êô?ÂÍ3§Ն?ÐëîʒN»?Éş؉)Æ?à›¿Â´VE?Ì÷³ïõà†?© Q2'f‰?¨É†š"X?€0…燤?'1üÂ×Ø#?í÷ú*±	?­ùÒÊ.?¾»ZÁdZ?Ç^añL¼?ʕ¡E6l?¿9ú³Ì?åƒ,Wb?ÉÈ]Jø?ən2…?®{®Â©;?³ 7Ñ$5Ä? úcÃOɸ?ç5²ªjTæ?±r©ÒJ/ç?Ò­"ØÝ?Âí"=þ¤q?¸ÑÀ˜>®?°õ}¼?ø?ãâ…?çÃë?Åp 7SºxOTHER3FGL J1839.9+7646@[8›R~@;ÅïbúÀ:po»y¾2À;ÿPïܹ¿Ÿ9%ÑÐá'@
˜áT@ld¿ó¿ã±Š#"ê`¿è¿|¤¶¿âܪ̃¿ï"wõºUNASNone?._™?€fL¡¬€,?h{Ž"æ\‡?e!5Ü
8?'½Ñf"?{£÷ºMM?í!×Ûk?°[űL))?«KiÔ½¯?£u–óá‰~?¢c6ßyÈz?¥ûDéÅÕ-?ì¶sõάT?¡ˆákŽp%?§Í¹x/‡D?' ˆC'w?¬Ë-yh?˜G£½é£?ì5M¬R¦8?¦¿¡g¯–Ð?¯¤CS­JR?žé?ø}$¥?­á㸶:?œ4ÏCc2?ïÕ ºØ?pÏzA[µH?_åahT?]2u´N@?jí3ÜeÅü?gïõpç•?ï;8s~?:ZbÚ½<?‹·H,ô½?3ýä>ÿÕ?…ƒ)¹¹~ú?ˆ3»^ß`?î9¬ºï»Ë?'›Û1È?Ÿ§ºV™
?‡ÏuÖ?™"®DA›?ƒ+œ¡mñÉ?ïlí­Ý?"â°-îœ?ði$ªÛì?yd3"MÍ°?†Y'~®l÷?z9L@
29AGN3FGL J1840.5+6116@VÀŸ±@8ÙìÔªàÀ9Üuι6À;›¤xð­¿èù+¥þµ[@´D¼­@۞ÿµ¿ë÷&~*8Ÿ¿æ:QB›c§¿á@Æ®-X¿ìªJkßUNASNone?ïÕh‹?õË?sHç°Áéñ?mØ5r:ø?m…pðh•c?Y~~_%ZP?`‹ÒöKe?ïV¢ÛÙýY?—y‰ð…?'36ï32?ƒüÂÖþ?ˆ$ä8?'æå/wÅg?íŸ9Ž
–¹?œ€ÿ!¶Ü? ¡
-õb–?ä>0üÈ?¥kYðUJÝ?"Ї¡²]Y?îPÌVÕ,?˜»Ys>*?zõºòyÇ?tb'§Îù?§"ˆm	^G?–äúßèZ?ïì"£ƒ?aŽã‰…?\ŸEðœ'?[Ú)3W~Ã?F6Ywd?GÊß;wc&?ïÊcüSÎ?x´Aý?gg{ä ×3?b–stw9?n4‡¿Òw?s܉d·t?îêw€™?ŠÉÊHiúe?'²¶ 8Ò?'wWùo?üÑûŸmû?€²'+Q`E?ï¢"2kl?sÊo¹ò
¼?Xj¢ÕgY
?NR']o–P?"j»ô?rŠZnØAGN3FGL J1842.2+2742@LÌݓÄn@,18yÄ<À9'íG–—‡À;|5vÚQñ?ìpRqx#Ž@
?çݟX@!¿mh¹¿ãMû
Qø¿ÖŒtšUè¿ßGDŒ¿ëÙ<\QºˆUNASNone?Þ .—ÊS?Èoa|¼?Ý|Îýԁ¢?ÈÌ«4 Ãð?¯UÉëY?«¾UºÂj;?ÙäØÙ\?Æ·³µúxW?ÚE¾—8™?ÂvT\Åö?ÈtºÎ-Ü?Áó¶E¡ÊÁ?äûVÇ{Ãà?´êpéb‰×?Ïfّ3ø?²X®Ò¯È'?¹W–¡¹ðô?¡§ët‹K?ß@Þ·?´5ì(»=·?Öil_Øò?¶|vê\æ?Ĭõقà?©ìtKÆè?äo×­•=Ù?Èsr[š¹?Ô¢Ðìäf¿?ǒ¯hY?£ëý¼õ7|?¡ÄpÁ_æ'?åqplñè2?Â6ǧÉÞ?ÌW¢
 ?¸Ñ8Éùrm?»Å8n[}T?¶]üàßÖ?êG-Âl1é?ªÑcPۅd?Á@1ܤŽÉ?§
!-VF?¦Œ\aƒ<[?'t."׬¾?æ¢Ò+Óe?§X­»ñz…?ÍZõQô?¦ˆÃÇÛ^?°5m6›p?"pYaù¢ÌMIXED3FGL J1844.7-1224@56q¬À¦žË1ÂÀ9Lx䓓À:›¸®ã®¿ÖYIŸ}«Ÿ@­5'Þê\@9*Ÿ»Ç—¿ée÷"þW½¿è·×À⯿Դûï=ÿ¯¿áŒë¨ÛUNASNone?í6Äsü•×?²ù|SÈý?…BA$)ÙW?ƒÂîI¿ý?³¡"=»×š?²Å+~'Ê?ëƕOªY¨?Ãb'K?'ãØÝZœ?˜œ
,쬘?½R_Hdó ?Á¦a¦ì›þ?âp:ˆ¥Ö?·Y8ßeBß?¹›…pÜ?¦ñY&Àg?Ôßl
X?´ûúM=¿a?è7³}ðæ?¿ÆҌÕ;?S(v°zJŽ?T\ù¼­7Œ?Îúáºö·?¿xR™wW?îqà›ÇØX?­‹æ‰©ð?…Þ/zàԓ?ŒÖ/¨	}?£jjdÊEc?«0ÚÞmŽ?î«e¥åñü?®5T–Gd?|†¯óª\Œ?ƒ²¦ ‰º?¡¸Ï£m4?ª†Ý%ÒÐ?éÓÙP5Cü?±N·@*{?©nL8è©Í?mÁ­¤?ÂU°ðŝ?­X·@Æ?ì>äûy?©6
EGcÀ?ZY±eªâ?K­­ãB?½¥¢‹"r?©	:ѸAGN3FGL J1845.5-2524@"á˜kœ0MÀ$(^ÃÚµÄÀ9]ÉòîÀ;*¾áQ¿?äkõö«‡G@
™•}U@N@A0ÿÒ2½¿ã©åÇù¿ç¢I-ÆaÏ¿Ö'ˆvîÀ¿îIt&(ÄÖUNASNone?Þ³•I¹îŠ?Ë@@LÜ'?ÓÏTœ9‡
?ÉQêл;L?Êú,4Ø?Âùߌdt@?Õ%D!ù?ËÌ@Þ ‹?ÖFãM[—D?ÅHH42rÕ?Ԟ÷nƒbÃ?ÅGÏyœÆl?ã'b d,?±íÓéDÔP?Ê0élj·Y?«—ïŠé
?ɌÍ·ö?«)]dAÂ?Ú¨`éœ2È?¹¨	'JÆ?ÅãXy¸V?¸ÀòMî?ÚeòÙâñ
?»'!a4ßl?å§çe)?ÇZ¤«	r^?Ë£–?ÃÔ.YÉcÐ?À\ŒpÄÁÄ?¸¶Ð*xš?áA…ÜÖã°?Ë+²U¨((?Ï»å‰\4´?À{½NR?Ë>H<?À_ŒAœƒ?èm'€?¬â|ԕW»?Â'ìÿ®\°?¥Wԑû?»:—fÊ¡?¢:¿ñvÈ?ä6•×~gË?²5§rn^?Ä4Vÿk/¤?©CÐÞV?ÊñQ¢›10?«Vž
TˆMIXED3FGL J1849.5-0124c@?v«%(®¿ÍÇø<<FWÀ8Ê<ϔ'À9}⊤3Q?ñÂãoPšÍ@ÕÅ©@Dàßÿ.Ÿ¿æ•H\mÇ·¿â‹ƒ&´(¿æÌdÌL8,¿ìFeXäUNASNone<?U'¡Þ`@?S,@™°è+?῔P7-œ?У )"?Ük°ZÙÈç?У´"M­»?‹ü€àj'?Ÿ&z›°'Ù?ÑuŸs3s?ÂD·]Ä?æÕ>Ce8?Ã0F4ˆ?±+µv?œ©ýw·?݅qü²Ì?¸\«ei©K?Þ4"Ù,"?·vN¥f?Ÿ†]~C$?¤Ðg©5º?¼" º¹éŠ?³Þ˜`»Tö?ëq;=æ?»'*[녗?7¥dHf?>è
6!3Ö?à•"Võ¿?ÒFÏUEà=?ÞÏÑñÇ$?ÒFáÐ-ï?—sÚž?§BíÈ<f°?Ó{ÀsUÁ?Á§ÕFT3?å¹F‡Æk?ðä»ù7[?¿.aÎb_?¥ÎË¿ñ?Úg(6?´yë	(Î?Þ©Q%?2?´€;"eâ?›ÃjSè:?©M/0¢¾?ÀÈ¢ÆœS?°F(†Æ~
?êï¼"š?ºhÅ«	GMIXED3FGL J1850.5-0024@@;ò<ÈÞ+?'çT¸i"À7"ºV¨ƒÀ9¦AÂB/O?ôÇW<§Ñ@¦ûjo	£@[?²r"¿Øò‹p¿ŽS¿é™Óêè¿æ†Œµõ3¸¿çÍ`|Ü8iUNASNone?s(
\°ï?u/
ˆé ?©7M"ž½?±3¹y™?îF>ªò?±"Ûi;»•? Ïzþ̟?¨²^ðýãÙ?À\ª¦?µúÏ<H?êÒ±5A«F?½
6M³«Ø?¶—‡²X°°?¡xÀèàK&?ÊÚ^)oÔ¾?³³d»×?ævw'0
?µAK}@˜X?²=ºQžN?®ÍŸÅ'ñ?¯Èbh¨õ?¢Æw†ña?뱒"4Ç?´¹ÔÜí•?y+Ãn?…&î	'ž?µÜ¨$ž[O?ÁX£ðÃÄ?íuJ&a?Á"ÁΖü?±Âó¶Âô?º¼ñÚÅ«=?ÆT£fL?¹5Ú/{«?è2`|n?źÌ+M?À¸¤ñ*hù?¦÷›|y¡w?̀l½Ô?²‰×PP¨Ï?ä±»"@>_?´vžÇõ°B?µHuŽÈ;`?³œMoཹ?¹Ñfÿ,_H?¢òXú!'?êÄn%ïË?¸Ž›BH÷VOTHER3FGL J1852.8+0158@Alk΅3±?âЀÉ"À77ûº !ÞÀ9Ã~ü_a?òýó¦*v¡@üäõ‹C@`Пëf¿å0ù›ü!¿ê;ƒ[6)¿å²Æç'¿é¬ƒIS¹™UNASNone?{M-eT÷¶?2ü‰Ú[?·_&"('?¾™}má?ì݀Òßq¦?¾ü¿¿Ú1K?"˜ãÔ4Ñí?¥oô"í?ÌÈ­¶ål?ÀÖt{'?è)
t ¨?Áb§•?´¥C-©©?¡žßr¤‰Î?ÒÛ¶}2¹?¶z')ã?ä\é¾±<_?·æì:~À ?¥Ô|ëWÀ?¢K_[҆?¾%'c¥Ÿj?©çÜçÖ?êÞåÆ?³®à¼Ñ~¤?iõ~Q&©±?p‡•.Ú?»Qhòek?ÃK9fuwH?ì{é"™)?Ã~¤"ÈëÛ?²]$ÁU?½Þ"î)$?ÒlLç0ȗ?Àmºá›n?ä~4ôSyz?Äžý(+»?»ø4{˜ä?¥f"K¶h±?ÓTáZè?µ`Áw¡O°?âÖ¼ˆÃÕ?¶²@µ"?«²•°T;Ú?ªýÛöPù?ÁRIKÖö¥?¦ÇV)þ?éðDQ¤ÉŠ?µ£rþFOTHER3FGL J1855.4+0454@Bá
£3v?õ¥+•°À7ÐÌ% †À9ù¡t?íZªŠF"@
:íO¤-@W— mˆÅ¿àï6ð3À¿épJÜ$â¿çNéWпèržïïUNASNone?hÏ>ÝÜw¹?pÍ>mÁ'?¸?	Dì&?¾ò§´~?ìßO˜ý`?¾fº…]³¡?»g‹:ÂZ?Æèô¤ñÖ5?ÍÍÙ|')?Ã;É´jW?å)R—°?ËZÙT"J?½·<Ó×^?¥È©)>¾?ÐiºÝû¸?³–tî:?ä:ö‡AŽ?µnšQVä?¬``Ý£OI?¥&Œ~?Àtç"DY?­´½å½ÚM?êÀtéÙ?µ˜Îêo$?`D±â?kŸ—ö±k«?¹;#¨·ÕÖ?ÀºÁ&ÑP?ìÈVÙ*©!?ÀÕð¯L€¯?ÌV¼ØÁ€F?ÑÌr£¥Oõ?Ά.­½h?Ã巙"À?áHÅ`Eî?ܞ»ä¿?Å:Íþw?ªö¯@Â4e?Ñ)íèêÿ?±¶ Vˆ^?â(jՋã#?³ä­Ølu?³¿Ø©—?®ó>cƒ+?ÂA¢LE¨×?¥ØŸW¸g?è÷œX)¦†?¶fŒ§ÈÐLOTHER3FGL J1855.6+0753@D7Æø@B‹`òËÀ8J¡!À:^×òš¼¯?êSrBèˆ@xrÊø·6@Њ©³¿æÚ¯Nњ¿é
X<Ï`¿ãŒ˜qGã;¿ïæ_4eYÃUNASNone	?¶Çê€`h?µõ,fù#ç?ÑtÂþˆº?ÌXí¤?äl¡13–?ϐÒQ,S¬?Š[ö;PÑ?¡-åO&c)?ä#¤þã±|?Æ2eDŸ¹'?Öå݊4Kâ?Æ'IEbø?DŽzÿá³J?°§ƒž!í?ъÏÄm?´~Õ@å?áYy±¥\¤?¹åP|DI0?¡Í[·¦i?˜i«ZÛD"?Ø°`w†k·?—üUÑmÆ?âŠúç|ž?Ãdr…K?ÀX˜U¦?À¿¡Ã+/Ñ?ÕP£¿Éj?Íđ2•z?áA™,XÅá?Ïr7ÍC7?¤ã†½&š?²œGìû+à?äÀ
ë¿Åí?ÀN8æ.%`?Óã^ô?¿½œ7!ø?×LSuró½?³r÷å8Û?Ε™Ú²·?¯õœŠöϼ?Ùhߝ4ç?´(~ЇÅÆ?¯ªéá›ì?¥2$ò&[?ձߢ"»R?·|â­>$?ã,p^G?»ç±výYÕMIXED3FGL J1856.1-1217@6whۋ¬Àf•Ù¸éÀ8î¾c}}ÚÀ:ë´¬D—	?ë«Ë<vJW@ofw®7`@¶?wå¿åíQŠ"̉¿ë7ú&ïzn¿ã€<"Åý¦¿Óm'ÔUNASNone?çþÛÈñ©"?Ä"´*>—ë?¿ö"`8"?‰ÅÒÿäÄ?Î('róVh?Ä
Ž¤´š?êäýºDMÒ?ÄV=³X¡F? 'EÌ	zÊ?¦…J§‰?Àb7¢Ù‰I?À¸ˆ†æ?溜ÁlFz?´–"`™ô?±îçÛ,GB?›±Ë®X‡D?Ì¥á¸?²˜×")x?åEÇw£O¦?¹ê!é¬#?š¤ óOú[? –ØýB?ÓÊ'1êo?¹¢ç`¡ÖT?ëɇÿ¤v©?½mòvÕtf?|¥‡]¨î?wT>l?¿ég'x|­?½3ñ–}&ê?îFé(?±:Iv<?Š—¤H›Ë?•Ñ*KûM‹?¤ùøiˆ¯¼?©µHY.?ìé>Óãu?£`ìë*z?Ï}«\°?Œa‰hç#?±B/6
,?ŸÓ¯•‡Ê?덍æÌÁÿ?¦·2 €‡?—¤y¥"ë?ŽJ"™ûÌ?½ªrb{¨Ë?¥ò¾ÒLä@AGN3FGL J1857.0-7341@t]9–ûÀ:W/˜sÿ¬À9¦ÃhŸýÀ;¢«%³ð¿ÌÙÑò?fâ@OüÄâ@;z¿ä±ñ¿é€ê&¶v¿élᄌ8ª¿ç؆ð'M¿ïÿaXNeUNASNone?ïÊÿ^´/6?wÙÆî?e"×o°ï?m›'Q§[?olœ•]Xû?n1qˆÌ¡h?ìâüz%ê?¶Xquj
±?¡Èt&AU?¢÷›Ë?°âØ<†?±4R
A€?ìúB R_7? ^o0–I#?©‹o¯é§?"D"3Í,±?¦Ð¼Œ	å?'Ÿêý j?ꆼü F?®¬ëhdÚ?ªe"B<? Y°¢) ?¾—VÖô?©Fàu\_?ïäF²Û£Ä?v½f_%ñ?Z5(7é?h‹:'º¬?]=rÄ.2?eèµpm°ò?îý!V³?Ÿ¨é'Ö6?ˆBÊTøTæ?‹y¦Îü?":p;õ'?–óo_§,?î–ÀÜÝÓ?‹d©|¥?›Gûí Õ8?ƒy\±d?'ßè|czd?{"¯'ýh?î°Â.'—?vgYcE?‡fš¤í›á?{HºÄœ?ž4p'¸ß8?‹&-E›[4AGN3FGL J1857.8+0129c@A€jüοè	_s­øÀ8+-ß6[ÝÀ9t°/Þ?òö&Û6@
ÌûìJ£@½Óà'Q|¿b7ž¤&ƒ¿ç¡YMp™¿çÛَÀçU¿ë9ì¡î·UNASNone8?S	•æם?T(ÊÞ7:?Ëm#w†ý¾?Ê{Ovà²?é2VЂu?ʅ̡ót? ÅŠuO½v?±Ÿ@ezº?Φ;™ð<Ð?ÁȞe—o¯?çJr<³e?Ä)â,|Ø?±·ëz?›Óí"P§Ð?՛º£ ùA?¶8ÁX¥?ãÂ
½> ?¶NJK3Í:?˜<>«©"ù? ¥´ŸBq?µ´ÃNÞZJ?°$0Ú?쇅 Æè?¶,U_Ù?2 þh'h?;½üÁP?ÈÝ 	Ð[?Ë÷³ç^ڒ?éÆcÜÉD,?Ëû¯'9C²?®~ÄÚy®y?ºKä\?ÐØøà¸"?Â+5‡e(h?嬶Ç?ÅØ0COò?½"¦Õ07o?¤±Öý']'?ӉðþŸ¨?²€›¿æ>Ì?−¦
k>?³X$_Sú2?–¢'·c^=?§¼ºÖ·?¸É¨ÐÐ.Ú?¬ë
¨ê?ì1¶X8£?·`'q•âOTHER3FGL J1857.9+7319@ZŽ4@9pJ¥?À	À:
ÍfOÀ2À;ö{í·( ¿ÚÇH¢õҙ@âÎ}Q@'R€«a¿è¢Ç:î¿ìzá%Qü«¿àj$׿ÑÏTŒ[áUNASNone?ïºô"mä?"­/FÁ?D¹;Ÿb6N?P€}:?Nv?ƒËc°D|?ïv­3ªQ?›[RI"\?~,"CÕ~?Ž']rèN	?ƒhʘ¹Ð"?f¯¼†?íÁÄ°ô?šC€EP:W?'í{Ófî?Üg7]ñ?ªì÷(°p?–²žÃè@?ïóoßó?'psó|@?aP‰ŸÄ]•?e©¼ïóï?š×€Õ´o6?'†á‰†÷·?ï´Rš˜•?©ŸÉ:¯?QšºNňÔ?y&pº7?€¸#'ó¶?¦Þ0(e¢?ïÑWܓqë?''¾vÌ?e_R¼^—D?t®Î?¶?iHÐéèí?ríÂõ`OX?ï+2q¨u?ƒI›{\]?]1n$?iÎ%Ϙé?'Âen-÷?
/»žï÷?ïÞI'2¨Q?g¸6ÅëX?B¢J»÷4`?;ïb(¾î?m
ë7]o¶?e‡R2Ù|AGN3FGL J1857.9+5549@Ux+Iº@5GÎÙ‡+À9Î.ümÀ;GþœR±?Òvۆƒ0@Ñoƒñfµ@°uˆ÷5¿é]h»L¿¿íŒQ=pŠ¿Ï||àØ¿Ô¼ÊJ*_iUNASNone?ïÄg~ûnÝ? fH§˜D?Jm|Í?KB-ÛÄÁµ?z~œ¶*.2?€uŽs]L?ïn¯[çv?™·r-Ö
O?~Ϩÿ{f?‰xÄÊ»HÃ?"÷¿žùÆN?'ØU"›­å?ìð½K"AÛ?¡ÜM\ÚM?—"àûd5?…Tî4t¨~?²±]bÍ"à?žûË|8í?í('QkF?¬¯L«¡¦P?}i€ ¶¼?ŠÔ.Ü[?´åWN•a?«"UæDÈ?ïæ_ËA²R?kbE¯¶‹H?=í©ô–u?@ŤB?çÙ?eâYÛø<?i‹ˆ_?ïˤ«gï ?'
¾|á?gm'íŽ?rœ®ãáóò?lîH[…*+?u"mÄb§?îՙ9ò¸?¿"1Iñ?…L¼M!´?|ð³g'*Ö?š¦z»xŠ­?‹zEoe?ïXOɅ´N?‰®ß&¾?ríøÖ´æ?lđÙ½?:£S§}û?‡BI£"‰ŒAGN3FGL J1858.0-5423@u`¢}ŠÀ6­Î|Ð57À:&:ØC""À;·¢Ëq'ú?ésÐ#eØ@
Aå·Tj@ô<ŒAí?ØU$äTÿÜ
Öfma¿é£*—b¿×ñŒÃ%ÜUNASNone?ïo­·ê?¿Çt«õþ?yVƼ	¬Œ?~â€(\}?‡q2ÙW[?Š%!ê¹ÜU?íc‡
rPÍ?ÀGd-?œ®¨åàñ§?¬ÛŠÆ;9ò?«p:¹Z[?¸AŽcÝ)y?íbãVži¯?œ¤‹û¤¬?¢9yÉD­?'"‡jV±?§˜PΌ†?'%œ¸++Ý?ç©û«BË?ºY_³Cd?ºäÅy-?··^5i?ÃéUÊvÂ?³cXJ1?ï×K'¾z?uYÎÿFú?Ym3—›\?bÉq_Ö	Ð?kþ>lžÐ?mÆX"´ô?ï)nWÞ'?§áSõ#Ö?'Nj<¥õã?"6=a†î÷?'ªÿúIþ>?¡$lð?îñóÈd2Z?‡7>´yÃ?'-V<EØ?€i)UxÕ?"ƒ¤¦ë?x£Š%‹¿a?í¡±ž6ó? (nä4)?¢Næ+¾V?•X÷µP%Õ?£Ö—6I"?"û¼–¢-AGN3FGL J1900.3+0411c@B×u}Zž²¿³'¿ž¢(EÀ8XU±ã<{À9ÈQÎÿ¬ô?♺™Cˆk@
Â/,"[è@ÆŸŽP:¿Ñ:8¦öµ¿è"[clÑ¿æö&Ó±öæ¿àK!2߄UNASNone%?n$˜*?pû8'–àd?˜æ´d¿Œ?¥"âþ!	Ž?ï¥Æ6Õ?¦7Èk¯Ÿ—?³†Ð•äk?¼O`cò?¶`GF?²R©S͑×?êÜlZTo?ž¥8ˆ#?¿T9õço³?§-g ³oR?Á(á¸8¸{?­ цÅ×e?çË@S4ãë?²™}5:ƒ?À^dÀ° ?¼ÛšI[­j?'Coˆ§m"?'YƒIt?ëVKSe'¼?¾`¦&"‡?hŽðƒÃ;ý?oI.[ØÏØ?¥>SOl֖?µèåM2t?ÚXƒ?¶#]q›ï?Ēé˜Ï ?Ëæštò4?º;Scæj"?°Å4Ý?QH?ç"Û-|~Å?Í X®?Ɨe†[h?«.ø×»?ÀÕ>`bì3?ªàWbV?æ$×Pjë?±þæ+?Ãge%.õ?À¬å­)ª…?›IЏ—:®?Ž4M¼*Ñ?ê^¢UwM?Á[7``à7OTHER3FGL J1901.5-0126@@f…ÂL@JÀ]Ç@›Ñ'À8	ð1UãaÀ:'%ž:X?ÝÜ背'ô@fÖ
hHi@ò'ÿ¿âül`(‡¿èõÐF~êl¿æ"&Bý"¿é¢ó*ë¢6UNASNone?á
fš`5l?Ëkdšb?±WÿÿÖÄ°?²—#¿'n?ُ2Ë·×{?Ì :CY_?Ó/…üP?€?Ñl_LŸHŽ?Ä1ÞÊPF?¹V8ˆó?áh0Š®¼Ž?Ðê
Ot?ÚúÑx¿?­?¸ãö{:ÿ?ÉYq‰7Õ7?°{î§Ùq?ØXu¤ո?·K™d??Öe]€['?³d"šªz?¶'
"aÜ?¡\%$9¶©?áûP©D¡?´Oq
{—?èC#Í~gS?Ç&W(l?¥svó'§?­0{jPù?ɖ"
þ	J?Åù"ŽV‰=?áb¢eßǕ?Ó®Ìb)üå?½¥æ}«…?¶9r4ÍR‰?ÕÑsz¡õ?ÐPNÏnº?ç3æ7
¢?´±5
C'á?»A2œø?¥ºö½_g1?ŏŸ'#zü?®Ä3!Ê?â]ú˜HG?°¹n[÷N`?°óܹ²q?"øMàÜÄÕ?×àG¡Ö?°tåCáãMIXED3FGL J1902.3-3702c@v~ᛐëÀ1öwÄ\»ÃÀ9¾'²˝À;]Öì
¶?òb̓ìÜ@
ÈpëÐs @ˆ/ž‹q?ãÕG§€ÚR¿æ½@šF_,¿ç¾™è7Ñ¿ï ÖÊÛ
¶UNASNone ?Òø®ãôÝ?Å<n›>4n?àYwŠÇ?ÉÿtjJ³?ȨÅôú?½#½Z¥#L?ÎSϺ+Ï+?Ä@'^$Ú?àä@[å®ñ?Ũý"ÇO?Î.Øc6?Á½ÚÁ'?Ýô…ÿÅå?´Õ|"—Š?×µnÔ¹€?´†Vß1iµ?ĬÞ̇5?¦|Á"õÁ?Ɔ[}˜öË?©ƒÀTÉyê?â&xû‡?ºc7¡µ?ÐoàLW"?´¾má]g4?Ûò–îÍ_?ÉYF¤Ì?Ü7KTÖà¼?ÉäŽ
ä?¿Xvõ»êŽ?³Z7½qþ?Ü|.þˆ?Ç-0u3M?Ø©7fžšŠ?¥᛻ݼ?ŵtÔÆÉÜ?»3"µ!_?å?ˆd¤*¨?²3Ófµ?Ð@9TÍ?¯Ë퇚x?µš»ö+d	?›mu‡CÕ?Øé:eEmâ?«ÓÇwTH¢?ܬ4àÌ!ñ?±TQÔZ¡?ÄÕ!sÜàZ?¦=ӄ¨ÅMIXED3FGL J1902.6+0655@D/Ù<FØ,?åԄƒEÀ8‰GnSš²À:Vgâ?âà:Üä‹Ê@áÊf–@؋Ÿ…ì¿?ïý—"ìпæHXT¼2¿âoO°0M¿¿å¦ÃQqUNASNone?ƒqIR¹?ƒëÅN;ìÒ?¤''"g?¨Íüî?ȟ?îqɁœUi?«§Ñcâ?—·[Y>¡?¢r~<Î?ÃT5nCKü?ÀunL_?êm7ÉEé?ÁèoâQ?Â@2;!ÐF?¨2úÍ<é}?¶¸zõÁ?£›WvîÑ?è˜ä—9ö?°2FïR³¬?­"WŸÕò?©GŽëûŠ?°¢QJ¶·¬?¦6ØÎöŽ5?ìp\«Éê?³û‰þLõÈ?…ZY¥ÿ?‰þ{øGE?šÊa™•@X?¢™Vqj?îՋŠ76?¥î•wà‡?¯=У¤'ú?¸~~ݖù ?ÇP˜ûVÄ?Á2rûÂ{?è7ü¶ýá?Æu‡è''a?ɹ‰µ16?®2}†s?µ·ª×:¬'?¡q£<wØé?æØ\Bԙ}?±Å+e*ô?´/Fæ?²öØÏdµ?°á‹Ëõc?Ÿ@üaŸ^(?ë]åÝÙ©C?·%Ê]ñOTHER3FGL J1903.9+0052@A'ʽf'À*ï9ßßÀ9O²G^cÀ:‡Ð|"µÝÀÙchÛ
Ó@ˆí$C@'& {±¿åšxBB+¿ïÇ>㕑!?í<F'Ej¿ãÔl~XuUNASNone?ßÑ=XêÁ™?ЕCrŠOé?hŠ4ˆ³g?q9 XdÌ?ßý®=âÛú?ТñeÍ(+?é×h'jZ?ÓwTt:SR?r´sGr?¢ò¡äêñh?Æ«>èH(c?҈=YZlç?àŽÛê;?¸¢Âô°c?²ÓœMù?¡Ár±»]ë?Û{4åÌ?·äá½IÍ?î/Òß)?º%屎ó>Á|Á¹Õý>êg›(ê¡Ë?¯œ¼àVӈ?º%þ?à6¶7"À?ÑÎá«g?dXé<ý[ë?ldÂXé€?ßiágÈ?ÑÔGùF…ÿ?í³¦¹ÎÔ?ÆP¸<¥€`?ŸûÛa?—37¢)?°4(=°?ÄA]å°ÀÊ?çeÙ_q‹?µi瀾g•?¦Ík;äçß?™<ô๪
?̵?²vž?³ É1ä]ö?ïcGêòŸ?›ô­ïðpô>µÉ±™+>Ðväþ!=Á?"–«'Ä"×?›ôp™‰îMIXED3FGL J1904.7-0708@<>iƒQÀÒWBÜôbÀ8'
DŒ!À:ä
ƒÁ¿ý¶3@=Ä×5›@²=@RU¿èØ(Ë{>¿ã@ãëªæý¿åø|
Ë"[¿îkìï.UNASNone?á¬ýaj(=?ÆwôÁ'
?ÒS¤áåýd?ĹmÒôâž?ĤÀ¶‹dD?½Ã'l–?ì ØxZ7b?À˜2ñïÆø?–ˆudC?¥«4tò]?µUZf1?»Ðã÷z?Þ´ËrÉdý?¸ƒw£¯?ÏoOApº?°UÔÂG_?ѓŒì¯b¦?µJäB[Ûx?é0Jàpe?¿.kÒzÐp?…>v¶eg?•™ÜÊÄU?ÉêíPøì?¾Ô‡ýÌa?çv¯´e?ÂæÉÝÔ?ÄCXøÈ0ä?»Ápx8 ?»ÃÑ)í~?·	åÐ₭?îÑ¢y6?¯¨'BÓ³H?=–‰§Ý¢?"7Bf Ö¡?,óÇñp?§yä
•«?æ6w|IÏ?²)¬q™''?ãB«²\?¦"\ÔþZË?Âßc'l«?ªeL{*Y?í.ûAÄ	t?«àNu3&×?L< VJ÷{?a֟bG$,?¶O­¯~œä?«ÏÊó¢²DAGN3FGL J1904.9+0818@DîE܃#6?éẃ}™À8̀eëí$À:&h!Q‰?Äw,S½d@û‰Eû7@`<`ƒxp?ìÏ7x¾ê¿î›æË{"õ¿Êï,ÀtÇ¿Ü}ìÑ
ZUNASNone?¦pГÿòV?¯Ý]-v"'?'‹RË~??$Éý©Rc?îNÅ«£åÖ?²G=å
–?"˾ə?ÍÿPۛ$?¨zBü©ß7?£tˆÀ'Þ"?éӗ݊gÖ?ÍëiÒÎæÐ?ÐF½_'­«?²BŠì'ë?°¢ª¬—ð?ŸÂրŠ?åÈLmÎ\?³)ïu©§?×30Pw35?ÇDîôŒ?f<Ñš?n;͙üïî?äPIšŽó4?ÇVQ–e³?"à¦Ä0ŽA?¤³¦"Ó·?v
GH	uG?…â@/˜'?ï,à;r$"?§ŠȘ?Ïn>P‡?Ôà¨#§Ú?°Udµ#~?¥>»8ŒŽ?æÃèo?Ó±†=yæ©?ÔSû1[?²ŽŠ»PÇ?±Ã¬mªÕ? ®k"äÞ?㝌ÙÓה?³œïeã?ߝUhÊK?ÄC×®…€?y¢Õ@…t?m"Õ_yv?ßþlìÈ@?ÄN'Š£ÔÓOTHER3FGL J1908.9+1022@F©æî·?ìJ¬áõÓ×À8T=ÚV"LÀ:1@\¢?óÒ‰šs@
£'䞥@®Ñ¾¿â^ñ¥™Ø¿ç©Õ7Ä+W¿ëΐÌEò¿ßº¶L5kUNASNone?h(rX@–?lïënþ,m?µŠJËÝ?½Òm —d¶?í6Ž45¼¥?¾Xœ=&Á?Äh°˜Ž­?ÍÍñhÉ©?ÂPR9}?À§ŒM£k?ækÑE"™6?Ϥ~"ÈŽ?¿/Þï(F?¥ÜǗˆç(?ÎøeEÃÈ[?µz»(?ä[êЪ
@?¶ÊoY¼ûB?¿UÜLéà?´!0.‹?Ã]÷.A©:?¾²¤íà˜²?çGwxåøu?Á1ÐIPx`?bÎᬅ=?lM•¼E?µ'¼×c ?¾Ú¥Æ6Õ?í<كO¼g?¾úZúwé?ÐÑ:¤Z›?Òí½2P	?ÂF9™Ãy×?½ì§f>€ø?ãÔGaà½?ÐÛ	ÛÎr?˅Îd°?®ÿ^L?x?͸àS3Ñ
?²œ¿ô	B?ᰇ·™ß»?´'BP´,Ö?DZ4üi¦?¶Ò0òÿ ?ÇàǓÛr5?¶*€ûˆº?ämÍ@˜ª?¿ò‡ShTJOTHER3FGL J1911.1-5318@u{sBí»ZÀ8Jt֐›À:&ÇÚÄçÀ;¼¦Ô¿«?óŽP:U~@
hÍ°LŽy@žÙ€\¿Ó3T·xì¿èx1Ÿ+Ì.¿î~.ÔÝ¿ïþEõF'_UNASNone?䀗ٿ¾?Ê·¤›ø'?Âä;Sh1î?¿K_Ë}Ó|?ÌÙÂM0Ï?ÅG~ÕÚ"Ý?Л3ßÍÒÔ?ƈA­tlä?àCÎz»¢?ȗ%Î>"?ÎĉykÒ?Áe*ÇSç?áô ûŀ?³€¦ð?ÒbGz_d?±W"jaë?Ãjí+7o?§l
÷/?È8ž'Ùôå?±¬"§í8`?åÙb(á?¼½:?ŽW¾?Á†þrg–?°ß‹<KÅ?çÂÿ}	|<?Æ_M(¸í?ÀNO:+?¼aúþ°Á÷?À¥³ÁÔæ?¼£°ÁçÉ?á´:ÎCU¦?ȨÅt,¼?ÓGê‡?F^?ÄĀz0?/?Ÿ?¸tª?¸UœÛ´
?æzò™²e?°8ÃÈÕ?ËjJ:?«ˆ€É3Ó?¶g™ç‰?ž"'ȁ?ݾG,©/?±*%\IÆ·?݇)ß`?±°ƒvÑõ?²ê;Ь#Œ?›=­G'ÞMIXED3FGL J1911.7+0307@Cº`Àœ~VG4À8ö}«ýIlÀ:·Ÿíp±¿ùMÛÅãúf@Á~Ëb@"éßW=ÿ¿å&5Bpם¿êE[–¿Úx+¸ô~¿äùõ§ÓUNASNone?êЏYÍÚ?¿ŒÂtóâ?€ýՑk£?><'.œ?íäp=»Þ?¿0E6Rw?èÇ㰂Øý?ÎsR-Ûk²?˜jÿe@ð?žÊô¬e?ÉÓR–Xz?Ìi","o?äl}ˆ°¬õ?¹7üɑDf?°¢¨µ¤
Ò?šõßY†ÿ?ÒþZÀã,?·Â:‡]…?ëÒÚÐ=%?²Š¿l‰?1¥Mù#j-?3ÿ%ž}?À«ÂÇTÆ?²‡³C2–?îrÃhÂX¢?«YÜ…ãã?l`›ó§\D?qF)IðLû?§
¿¸ëƒ?ª§¹¿j=Õ?íÿ\'Y?Âr¢èUr?Š¾n¨8Ê ?"'œKæãm?´z._Ýã?ÀpC1á'?ëáž!…?©^üG‹E? j"Á
ðÌ?'Ï4À'åÄ?¸½Ínqón?¥¯xnŸÇ?î[Žàqß?˜ë¸£´ g?"A™þóS]?Ã#Os	/?ª3åx©Ú»?˜ã´\øÛGAGN3FGL J1912.7+4610@SJ«Š\å´@/‹ºw_²îÀ:>´~!nÀ;Öq»g¿áŸoã×o,@.ÁÕøÅy@‰àiÝ¿è#ðÿ㭞YzxJ¿äf¨6{£K¿åðËLD&KUNASNone?ïÁº™ˆ@›?‡CâáiÅt?_Â6Gšk?ió"Ø®É'?w2%½7A?'êÙÂôoË?ï!£;·nÊ? ë'0àÇ?vnj¬?…5ôC?"4À øæ?›ùÅVËc¢?î.ð²žçü?"ùÐ(0|ž?"žÈsÿ»?¿—F6|à?£Aœ"€d?Ú
øȏ?î³bÝ3¼	?Zp7@K.?xŸ^ÏI!?nŒNd?¡µæP]cÔ?Œå ‡||?ïÞ
±M¯$?—BÞ)Ÿ_?RÐ6
+'?vü+o§{,?hDÒe
±?'Òkp‡À?ïÂåDŠ@?€«ýº¾ ?ehãhψ"?c,~­ÁÙÿ?sØëë«G2?zÞ©ºÃE?ïBŽBM'j?…v˜ù	"?'¦VºÐŒ§?vE…¤{ì?Œ¶©Èð?*Ó_Sô?ï¾ð²?jž¦ ˜¯?WÖü;¨_I?D·ò#ÿ–?{·ùlÅ&?h¯æZ
úAGN3FGL J1917.1-3024@4¹£$\×À2x/øìˆÀ9MG8£µÀ;d¿1ٖà¿íž÷ì$Õ@¤[«Ltx@å6ÿñga¿çù@Éì¿âÎSEÞlÄ¿Þß4½eÀh¿ä$×3"=UNASNone?ï`‡ïo†m?ãe<07?hÅ¿•·L?f»®ŸU?Öa;¨Ns?§ÍvÜNw?ï
œüG?¡……bñ`?|zû"?€^ç-Ù}?—ZoÜд?Ÿ2[ßß*?íÄ:–m®ô?˜»Ê…š•4?šk,ˆoä?†õT¦+•ˆ?¦†ÀT¦Ñ?'lgB•?íƒ-«x®?›à$³âœÍ?cìjŽI?`U)·8Wâ?³N[@ 41?›ŒÂèê²?ïàL"`Ó2?gT8©A?M¨L@à†?Gþf5)?hIX°—?dzªHoÓ?ïµoü]ö?ƒX{ME†‡?b‡;º"…?`'¤P|þ,?|dktû"?€È=gßT?ïGº)î!A?~ˆ˜K?ƒ»œuWu&?q¢ ±XW?ŠUÙ	øЁ?tµ³Õ&Üç?ïU'²µ½?{˜|%Âi?G º¬Œ?>
}<Mÿ¯?"—mNÊÙÒ?{6ÍO/tAGN3FGL J1919.0+0452@D76z—À¡±–¡À9!çû&|lÀ:½;ÇVkG¿ÆUm*QQ@2ÁÇ`&@Å'ßÂó°¿á•·*ã¿îIîª(nD¿Éy_+Mz¿åIĸ3ìUNASNone?â÷'áC§J?ϚT+Ȩ?|æܹ@?€£lrÄ>›?ٝ>Í£¿ì?Ï¢(£&$?æ·uUJ=?ѦÛ)9'Ñ?¥àwš-x?¦Ú¸§3² ?Ñ5u>Ö?Ð#i~@D5?ã^®·
?¹mÙõV¯?³rVÐ? L-¨uM·?ÕÀ¿Ó2?¸q¡f+Rö?äicìc•ý?Ã&;ú"?É?rHã*Ք?rå'éó¶]?Öäóî!0?Ã"ò7.YI?ä°9¾ßò?ΑðË&s?pžÿa'ýz?zÁ5k§?Ö]KŽãv÷?Βꨥó?ì¾ñFQ?ÆÔHe¹1(?"Diø}eî?›¤«ÁEw\?ºèíó@²€?Ä 54j?å?ê*vþl¶?®y¦g»Ù"?¤I:ɏ—?"øáӚu?ÂEkq4˜?«i3?¹'?ê(‹3A•?²óúßRã?xœ«Ì;ø=?h€‹¾Ø?ƘíÕ¹Ž	?²·à3_g"AGN3FGL J1921.6+1934@JÝdob@'T¡B‡À9,¶5±'µÀ:©-Ú-Þ?ß6ðôfÞ@
òA›«Â'@òÛ¿®×¿ã)¯–Á¿èÚZ~%Ë¿åw‹Dl@›¿ìÌx('2ìUNASNone?ÒÍ£
uh§?ƛÕðŒð?әóŠs-?ÊÓ;*<Xe?ٙMê?Ì#lI]?ÞäÆGf_Ê?Ѻ÷•í?ÀF«Bÿ'?¸ØRÌʁ@?Ø÷ä— n?Î%Ø!Ëå?ÖhÁèö­?µÅ‡ R-e?ÏúòÒ|¢?²ÏK²O?ÙöÕK?¶Èø)Ðf"?Ñ÷v¬?¼/`.­¬:?¼Q"<ŽÚ?¥(Ý9™Ž8?ãztîð?¾­
5›?ØÉ.—ÂÿÄ?ÊÑ`ÛY?ҜEWÅ[6?Éäë1fÕL?ԚŒŠ…Ä?Èéo–w‹?è]a†9?Ìd9ۘíw?±úÚaç¥?³•mÐÖY?ōoù¦äJ?ĉ*Üøi?âN^K©v?µèC(`?È>Z	GÀ?­åÏòoi?Έ,ȱf?±Hმ´?Üdñœ:?ºßkߎ?¼+%PO+j?
̯?ÜàѺOû?¹€›¹ÕMIXED3FGL J1922.2+2313@L'Õ'å!W@B™ØƒºÀ:CĆ­-ËÀ;nÏM°Œû?Ý[ò¤ÍªB@4˜³•™/?ùÿTžè¸ç?ácØl"&8¿ìl‰‰3Îl?åD\Ñ<H0¿ºhkÎUNASNone?ïyþ®I?"ZdJcm¼?6-^Õã7;?7'4Y#Ú?gzV–[?"5çúlñ…?åì@³#ƒh?Ö,QRêô?™@"8Ä|?¢ˆh9'Wb?Җzið	?Ôއ¹P?íßá4?¢?TíÈù?'&¥C6"£?€Ì@Âá92?³=‡·'Hµ?¡
– ¯§<?îÏ¢;mƒ*?¨˜€Nx?4,ï5·Áb?R
è<<5Ù?¢Ý'hÚÇÓ?¨Žì|Ìv"?ïÔ3QÔì?x߃¨ªz[?0Í(ŒJâ=?1ƶã'Ê?tلù¼?x2¹î2»?ë
àš˜?ÐË`Äw$?'?WG©P¶?ž"£
†–³?Á­Ñ–Øk‰?ÎI"ð"Îr?îÉ(2N0å?'{%T>?ƒfC(u?u¼n(Eÿ?'¹RCÊ?üÀŠ"$?ïÇ}ÃǍ?')rf»%?@'®¾ˆ?Jz"8'î?ztŽÚeG?€±äHVAGN3FGL J1923.2-7452@sÿ'}keªÀ</Ý÷vÅÀ9ŽŒŸ5À;ª­œ…Ý$?Ûs!ëb90@mdÆ~)&@¿¥`w9¿äh1à«Y"¿æå"Ód—¿ÚƒKÀY>¿â®xŒ6bEUNASNone?ïåpRJ?aù=óÈe'?FkÌÞÚ¸?DP×º?dôþG­¹m?_Ì°*&Z?îÞ¥'KF¥?¡sììêÞâ?'IlkM²?ƒq]aAOâ?›—ˆm-r?ŸˆÖE?î±é纹Ð?ºÏøï?Š°—*(ž?v±ôP$?œjtCòé¯?†²^cBž?íao—E4? 0í(z*?ƒK­{Ä^¤?Df8z"?²‹
–&ٚ?ž"b¨@'?ïð&VÞo?'">žjF—?9÷å4»´"?=Fšù¼Ä?Y5OKÄ?'!õˆÜÄ?ïŸOúÜ¢?†o|Ä>?k@åO`–?g<DŸ´ß?\‡ÜQ?ƒ.;"»g?ï‡ÎÎY¿º?qÐl3ðËl?wr
ö%Ó?aÞÍI¯)ƒ?'S=òƒZˆ?iÛGÆ1Œô?ïQÅ,ot­?cÚ=vI³?y
"ö'w?c§Õ?ëHT?zí"Ӑí˜AGN3FGL J1924.8-1034@;("ƒ‡ß]À(V*€JÀ9ÓôzùÀ;7›~v'¥?«x¥"éœ,@™Ã
+R@¾¦ ™@¿æ'H"¬:¿åÆ#aÃ¿Þ¾ø+}æ¿îÁç«lÍ*UNASNone?íx³ÿ™?° C…½y?«æwÞQè'?ªô½:_V»?™1‹$nœ?˜Ô5Hw˜1?èIÈ3Ž?Æic¶áå?»Øþ…gÅ?·_‰¡î–?ÀìÔx¬}ç?¿:ª®'?æ±ç¼h³?´Ao·`
Ž?ÅîŠ?­Ñ~Ouºë?Àr‡Ã¢?§ªRQñ	N?äÅÃìÜë1?´È'ƒ¥?²fu'zÜØ?¨öMßê?ÑÚÚÂïI?³5Dz®Fû?îïWˆý\?žYu8҉™?˜¤~>·?˜™æi?'á!³¥ÿš?ÔHn$.?ìïjj'?¶¿9Éߧ?¥Éw«"Ò?¤t[Ðõ?«?çPЊÄ?®>µ3P?ë6…^_m	?¨Š%[¤Ùx?·^DLÛ­?¡k'ƒH6Š?­Û!'¿_?™·ò‰ë¶?ëEnÈúI!?¢¬Ë.úÛ?¡[oZþw?ˆt¬oø?½&Ò8à;?ŸÅÞ1~F:AGN3FGL J1925.4+1605@IŠ3:}ª?zíݵõ'5À8	êâa‰ˆÀ:,îÉvÖ÷?™çÿûoÅ@µ…7âÅ]@À ý¿âî‹ÊŠ9¿é&¨¨L²-¿çM=«mh¿Ýü3¸ûDëUNASNone?‡A2 \Û?Ëmª'
:?Is¼eK‰?¥÷¼PÝûå?—ejq?©e'W»:Å?¬'æß×óE?¶%>:
È	?·å…öç?´ìɈZé?ëV$ázš?ÁA—~7¾?Ái¥?¨5˜dѕþ?ÆÂÌ1¶P?±¨uµ¦Ïê?åõ-N±ƒ?¶Âáéù?ÉIΗʃê?¼Ž×֍>?•ïNk?'¦ãàãз?èþäëå?½'úW¹>>?"ȧaö7?œáé°B?¡~ϯø?©ÑiÃ×Êq?îI²×êHo?¯
¡$Ŋ£?Ãz'°Àt?ÊÎQÀ´]?º6aâ"UK?°ëø 	K?çôU9ÃE:?Í5î¼F¤?ÏqëÕ¦"?±°ì*¤Þ
?ÅÜ_ǐÍÃ?®ËοÔv?â¬m;˜æ?´'.@Z80?Ó£º·e?À—÷‡OXò?'"G£3 ?'w«ÑE?åà
0a"?ÀÈCŠ27OOTHER3FGL J1925.8-7826@s¾ó¶E¡ËÀ<@ýâïNÀ9¢îš|îhÀ;m溴œT¿´[jƬQ@
¯G·Ï @`aꁿê4,s,À¿äøã5U€¿á–"ö¶;¿ïÿÞ$8 UNASNone?ìrӗ}q?¹²K…ÿ?ŒÄ‹jNJ?WpL×?¸Ö¿²±¯?¸V¶›ãï?ꚝ;Jêñ?»ç2Ýwë?²€üØ)ãƒ?¯ ­MU®?¸ªL4êv?³à" ³Ì?è'ÔÃ]¯«?¯¶×iŸ0%?º²U
‰¼"? ê[wüº?À['kÄc?¨åþGÕ<ï?æ<ZK€a?³/lnÝ8?³ÖìòmW?¦µv'¦A†?͂+\ç?±ÿù¾Ö?îsӟ­b'?¨YѹŽ?}tu¨
¼?~v/´/t?¥7S*(Û?¦¯5ci¢?î1‹Ù9B?¦l1þh3?™h14ûƒ?—¤ª˜Bø? 35kڊ?žR¯3抯?ìÿG¹?¡¡bΝ?¬aeÍC¨?•×³Iˆ?©¾¡>h@g?–¡©/$5?ìa8Šh¬Å?œÙƒÐ•ÀW?ž‡ï«§–»?‹±6kÐ?µT?ÃŽ¥?˜ÈlÄ8#"AGN3FGL J1928.4+1838@JÓý`éNä?âz
w·Ç'À8‹iŽ9GÀ::
fðÏá?Ղë݉2™@
ÖLØ À@S%?ªá?âPîû¿èŸÛð¿è³ü"±E¿Ü3?_2âÎUNASNone?ƒþ"Ê?ß¯Ÿâ«S?¶¯ â2@˜?¿‡Â#ð?ìÞ‹É­?¿æ~àÁÝl?±ª¸[Úª?·Ÿ¥b<Ŋ?µßæ²–`?´"ì‹{k?ë¬g°O?ÁÃîŠjZD?ÅӘx²C_?ªØ]kj?Åý]æ\A?±CëªF?åÂh<KØ?¶%)¿/ï÷?ǖÕÈ?ºWM;>'Ø? &ìv1öÍ?ž'¥TOòã?éu,þ?¼ÔöM4ø?†"Êópßî?"Ó½…EÊq?°Ž
،y?ÁØÇƗm^?í"ì$±?Áíƒv}Ç?Å.ú½(Œ?˧ÕÁu?¹–Ï9v‰Ã?±Ålák?çgiyHõ?Íܜ/˜ki?ѺŒêoÜ?±ó{^w…?ì"'üòY?ªa!õF‰>?âˆˋ|?´$'o2G8?Ò§ÀÇ8–Ó?¿V(¨Pþ?š#VNô¸W?Œ—¨4"E?åÛé§V¤?ÀÆJtèOTHER3FGL J1931.1+1659@JBeÛ
Ø¿è…uŠÆ—ÿÀ8›Âª4À:DÏkã}é?õekÒa^@žûo! å@üN¿ÓÀ?ßðÉæ,^¿ãÌjoEĿ麃㾛¿ïÿA¡DUNASNone	?mØâ4¶®?lJ[#­PP?ß €Iw©k?Ïf-ÓÅ1?àQæù/¢?Ïý©Â`?vÊUTjma?–Ù£—@Æ;?Ù/¢Qq?ÂËɹê>o?ãDê½pí?Ã>5$¤ú÷?°`ÿo'+?›‡*ÉZ¼	?ڶ͞¦@=?µ·káo?à˜yB®r¼?´â•jm®›?§²EI µv?œ†´ûÏã?Û´Þ©™?ÀTZ‡r?àªlV¯(?À"¬ãoÉ?g]kcxçÈ?m=ˆu©«?Ö¼HB€j?΋¬¬è+?äŠ~s£eË?ΛձÖYò?‰¨ôŽ.?œn{úƒ?ۖ0ÉKó?½"fSñïœ?áÎëlí`Ž?À!V;Bn?³ø€ñQ?§Ì'ãÙ4¸?ÖAßµÿù?±¡<7ÿ?à2ÿ ?²ýîÊ ë ?³¯·­Ê¶Å?¥Ùï-ÌvN?Ù"Œv4S‰?´B3má?àøÂÏGüC?¶-¥4uOTHER3FGL J1934.2+6002@Vôå´$_[@27Mœk2À:Uî²ÑÀ;ö-±l¿Â†J~˯c@˜zãKz@nÿg(Ù¿ë³e"®£¿ÊlLJE^¿âð´ÁúG¿äKR6·)ÖUNASNone?ï뫞˜ º?YOæìägo?I12:ã?B IÅ?\) dÈW?SêȜw«™?îŠ}× –?­üa7úÙ?"^)ÂK]"?—±Æã´ë?šR4Џ±?¦ô‡Ž²¾?îÃdfº|Ç?ˆOk8Y'?Œ!œ0B€?wŠÁb'â?™'¥ø!-?Ñ#¼"•?í¤­š"¥Ë?mÖ@j³? 8»÷²?'XÖ#ñHn?¥|k<bQœ?"âi®å?ïù74'W?@6%.r?0
«ggl?&nc<üIt?C-Š,?:$ØU{­?ï ™Ûš?[3#æ0˜?s‹FO?s…G¡+»?|i§Óáñz?ˆfEÌkg¨?ïs÷ªà­™?s¸öæ*³´?|ÐaÎ ð?g¦'OÊ*?"™äˤ·8?kJƒO3þ?ïB5ë°y?xUà`BR?|©(ñ!~?fî2ËHÜ?ZÞ
s^º?rP½D]åAGN3FGL J1935.2-7924c@s¬Ç£˜ À<£IàâiÀ9z¹9r•À;J›'§å?ä1äèç#@€9'ù@|#ꬿÇI(]ANª¿íOŒ³é7M¿ãÒìa›."¿Þ$Tý¢UNASNone1?ﯹt3N?'/œû£ÏÓ?`rŽ"û?bÖ®"Ñ¿?éþÏéãº?€RÒÇJõL?€…K"?«'æ1¤r#?…W­¿ªö?'"÷Îk#?žÅUñÿ?¦¬|eÐ@)?ìÒèê²q?ŸØþ.©? "|Ò¾B?‰)ê.ƒ?±&z?X§Ù?™Û{¬Çê?è±ßê?²â¯ w@j?—žI •³Ç?–ÌêÐ?ÌÙoK×Ó?²6¥á—g?ïޏR¡k(?l¡¿›Ÿx?O¶øU"?Pë$Äå«?i¬ÿµ©Ûá?gˆ)Ë{¢?Rª6?'ž)É"7?qŠ(uZ™*?z7®tH|?"•+fYR?)'PóP?îÆj¾Ëé^?Ox'é4?ŒêñVî?€m£Uî?˜½/t,º?ŠJ'+•?íg'ôæœW?˜>ɍ~ãs?'^Ƴ"ï©?+,§Éu?°o­º/^?–bÑe˧WAGN3FGL J1936.6-4215@vJ¡BoçÀ9Õõ'^éšÀ::7yéÑÀ;³¢/jP×?ðº<|]@ò¨ À€@w)¿ìêz¿à
TYôh¿Õ¬¿;>Åc¿ê¦;Ë`ˆ¿ïÿ…'yåtUNASNone?â§rÊ*?˂èŠw?ÙOJ$Ö?ËÎ~†Kf¹?–/<øf«?"£%šªvó?¿¼2Ò4?»§A&TÂ>?䋵o°^y?Æå!Š«"?Íó@UkÓ?Áß²ÇVÚò?âaVª=Ô?µ›ùl,?Ò*cæÚ?&?³f{×Ì6"?Â%݈Še?¦ë~Í<=±?Å
7§r[x?®Eé¿Ýâ/?çVsVä¾0?¸I_¨-Çi?»1õùõWŽ?©£Î™0\?æÒù·'?ȅ²Gć?ÒEïDé5†?ÈMa¿…
?˜QP}çz?"2UĀî•?×sòÑ`õ?òޕˆN)?ÝS
æiù:?ļ½I;?ÆqþûK¡?·¬úcü
?èúìV>?®:ÑÙ§?Ʊqºàï¢?©~ÊŒ?²UE$ùéÎ?šåoÚ#:?Ü^ù©¾nª?¯J½uy¦?ÞÚýJ ¾?±£ëÎûQ?³$.Ë~ö?šø[r¡ÆMIXED3FGL J1943.8+2518@NœwškP±?殧]Q"ÈÀ8ÑøAÆÀ:œÁ>#Q¿Ï…·3@
›WœŸ˜@Ó0?ß|¿ß	-#,]Š¿èwu[»e¿æN¶¶#׺¿ä‹oVÇYUNASNone	?ƲõêÔ?ÂSˆ Þ1?²ÿ'÷tý>?³Ã^Q(˜?çó†Ã[½t?ÆwȨœ?´P=3€ú«?À¥ïµ+?²›œöÕ»²?­½^®Ë+?ë""ºÂç¤?Ä(8ì?ØÖ¥Nê¯ó?µ‹`]ó,0?Á8èß|ý­?§ÖMêº×?ތæBi±õ?¶ØHŽ¶¨?ÜAY4,`?¿Ë
Z°?'ý·¡"—2?†'·üPàþ?áGe©@ðO?¿ ސ¢-?â8 O3x?Î1ÑzA˹?­Jϓóß®?¬™Ä¸†b¾?×å§ÌY¬¼?Í|–î2fô?Én›ä3?ÑX凜υ?µHщð»1?¤äÔ^C|?ç
I*Ý?Ñ~¥ã?æ|ä'Ê?²±¯…×)?µÆ[ëúi²? Ï÷Øèò?Ë,nwEˀ?¯ÀÈ<S‹?ä"yheˆà?¶u'È,
¬?‰™õí}S?tÎ&èñÌY?Ö
E ÿ6?¶.â_%í_MIXED3FGL J1944.0-0535@@óò^VÍlÀ,u\WìÀ9ðáù"»¼À;D"uuÍâ?К"»Dua@|Eëòè@ijàֆ¿æגMŸð÷¿ìð¯fEÀ¿æI8̶b¹?ÝڜÝàŠUNASNone?ïÆ2Èîà?}ê¨"DÞ?S'‡r½D>?W`›3•3N?xù¿Î$y?{uX"
5?ïg.'§¡‰?–'Â1_ÀÒ?rk2¢mil?'#'Š;l»?ŒþÂ8*[!?'\sî]m?í¯ì'?˜L Žx¦?–;:Ÿ«Yõ?ƒçُž.,?¨·pÞÔ% ?"Þ֍ám?î¾ö?·Ðç? ¸~Ácþ{?@²»‰õ?YéÿgȞç?£ÍÑËit? ´
*¯Ë?ïòù…½o?[_£m3Í?5cQ31?9L˗‡*­?VoIf¶ÐZ?WÔ'o'­j?ïÍÚE}¯û?x¦¡ö?ZkÞwÓvä?^þ÷ö}ì†?rwå¿_ða?ra€V‡5?ï<kÓZ'
?Å´
8üº?ÊuÑ0¾H?o_"ž˜`?•aäg?}™txÍ?ïÈJy¡?u'ŸȨà?*7+ '$?=È#Œé͝?{"ºœHøy?u`B"uÞòAGN3FGL J1944.1+3919@R^ÞÁÁÖÐ@V:ADmîÀ9Ý|š…RÀ;€½I¢¿Ã‹
¯ëëv@
,"GÓ@yğ»¿àôõG6¬¿ám5Ù¼Ûy¿ãä$3¢*¿æn`I°'òUNASNone?ïÀ‰*W?wÐa$²ºÆ?^ŠJ¤Ä?^žšðÐè?x[´QmëG?t*O.È\©?í®hºËæ?µ2DÍ?ˆ IÖ˙À?¼b˜çÈ?¯çëÞ.?²÷N!=jÙ?î8'g#®9?–‡=Nÿ'S?"$xÛ?¡¹²kˆ?¢ëÛyƒ?':K'.a?í³%š!"?"q‡ÍS?Èåsw
?r|k¿£dæ?°-¶Ù"?'8³¢D¾?ﮏOhÈì?µû\qvä?sÊï\<î?©3Lsü%?tîFFAÍ?¦‡ó'J3å?ï_Ú±šté?˜¡d^çQ?p£·"åý?q"GÚ-H?·Ñ¸ÐÞ®?•W^ÂÞ*?ïf–N$j?}|$šêT?[ÁL:?pßñZjl?†Ù¾ü\4?s Sɵþñ?ïd¶QÏð2?t>CÐkë?jÐk¶?R«Þ`»?'ÔƛyP?r¶‡\ÉcEAGN3FGL J1944.8+4300@S3¦µ(@"{¶NGÀ:Z©D1ˆ8À;¯¾ÌY	‡?ěáµ­E@
uËc–'t@!¿ím?ïæ"GÂP6¿Õ{è7È¿Öü}ù™Î¿æ̟m™
¨UNASNone?ï¹k;áá?'5%õ\¶Ù?YŸq¾¹X?Zê•t?|⹩r•J?€©%sÇõ?ì_oÚ¶ù?ÁåT5¿Þ? RŒë?¥Ð}¦?·øþ.Â?½KÓEÀ\?î"ë{Iނ?—& PK?'¹öY®µ?ƒb
âþÔ½?¤tMÒï]?'ô·ÐÐã>?ë¯XÖÁÿ?«m5\Šç?¢ÆЅ$R×?•†%­ë^~?¹$Œ÷%º?§ ZÄjÕ@?ïìÀ? ©Ù?cƒxæˆÅ?>µÌ¡˜1®?=اfy
ƒ?^Ò
óÆ?a{år@ÕT?îÈmŽg¦?©¹ÿË¿Àý?‡l<.Ó~Í?'~–\C?›<0
w<?£F;|òˆ¸?ï4X&)+ë?"Ôßjß?ƒ–,[¹sY?tÝ`t9ö?SÊ
œú?€jYÑág?îºQXžbè?‹Íþ%Æt?ŠŽsQ°?v	…"ø?™,¦±È?‡ýÄõ ²AGN3FGL J1945.3+7329@Zd¾ß¤@@68üPHðÀ:4i¼\<AÀ;µò×s?ð9»þHoÛ@þ@ô'âÁ@XY …F%¿á1ÆT˿룠ÞÝE–¿âÔSÝUd¿ïÿ™`Â@5UNASNone?îÂõúSÔÐ?¦xHøyÔ?€õ$8%VÃ?†D^0ì€?Ÿ&®"Ç_µ?¤T×wê€?ß-²€E_±?ɉIÊú9Â?Ú•#Ï?È
pœ-?ºá-¨•ò?¹qÆõPS?èRYmsdÀ?¯÷R)À@?À»ê֑áX?¦èá^(?»õ^âõ"R?£r•ò
Âþ?ހ׌ª"	?¾}įzŠ?×ø'úÇdŒ?ÁP¤C|é?Ã
,ñ.×?¬{ôtþ?ïUÎýdÖU?™?¶ËÄê?yȯ[Å?~%k@ãˆ?ý\R4ò?•"áÂÔÛ¢?çýVNãŠ?ÃøÎø	¢?Ë®^ |ëA?ÁØrÝÃ<?¯†°!kP?¬¶g¾QË?ëÓëGWL?£üNŠE¡q?´,
f̗è?œ JBï?ªi6ÀÕtp?"MD"Ü%?å­ »üé?°—ÔúAé?Ñ¿–‰Õèf?°ƒà(W¼?§1?ô#ã;?'â'ø8ãAGN3FGL J1947.4-1121@<æÀ§¨À1'äy'¼À9À=h@[:À;coF߸b?ò¼¥¸5ç@
Ê8ƒW
@9T h«:¿áã¼üS¬¿æ[Ëû
¿ãàý·©ê¿ïÿÆòmESUNASNone?Ôo™?É!€b³K?ǒÑ7"jw?Á³;´¿˜d?ßlja=1º?˲(&Ýh?Җ4x
[V?ÄZ¦K¦?Þ2é"Ç;?Äïᄔϰ?ÎmÄ]DÝ?Á"fP/Ý?àð›`:Ÿ±?³P0›³&?ÑêINApR?°…±‹¹î4?Èhÿ⒠›?¬4vü"?Óv0ÞÅÕ?³=¹Oþ?Û3:®Ác?¼BÏrO?щ›æŒ!È?²2½E?áDp "¢ð?Ë
pH‰Óö?ÂW¹¥Rµ?¼sRnHY?Ôgòâ$Å?ȇªµ1
ö?áö÷<ÚHX?Ď$	coÖ?Ҁ g˖?¿~eûKT+?Ã"â>_Gt?·lœ"4?èNR7I1?¬âúègR¸?ĶÑz}ìâ?¥Õȳճ?¶gêz%ñ?ž_—Ø2ãU?ߣÅOˆ‡?­¾¹ð™^?×ØÃ'SùI?¯B'›üv?ÁïFÿn?ŸM{BMIXED3FGL J1947.9-0743@@0,ÂÖ©ÅÀ0"ý*bªÀ9›A<á1ßÀ;WæáK	?ä]š@ÀgŽ¯…¿@= ˜ò¿ÅfÈ/¿éԇõ¾nÌ¿àiFî?Ó¿ïÿàí¸w"UNASNone?ïBtm?¡Õpkj4¼?P³Áùã?†ÀµOH5Ð?•/eªFž?Ÿ²µÂ=S?é2!–¹Ñ"?ÂG"úçù_?·ú±Æôm?±š«Ò×'ð?¾tA…ÜMs?»…鬊Ê?é‹@FRZý?¬!3ê-Õ?½IYµue?£¹,©M¹?¶\årmØ6?¢®'(·?äì£À )è?²8q±T>?¹ð";—?§×¢"Gúu?ÏUl¹;Ë]?¯MÚW¾œ¢?履0(ß?‰BmFǓ?j"ÎRF?q *_£Ñ?(Ö÷g¼è?…/Pûp#T?ìÂ@vŠh?³–¬I1'Ã?¨OʙpóÁ?¡ò'ºDnv?«Œ-ÿ¥c¾?ª4(V¯eé?ìjž{Íù?¤YÀŽ¦?³h*>?l…'»(ì?¨
MF^ýõ?š1ÑâŸí¨?êé»ý5?œ†Gwûɖ?²³°8oò§?"I&bàâé?µþoߛbp?•sOã*!áAGN3FGL J1948.1-7059@tE¤Ý/ À>#óYÿO×À:8	=–c"À; ±Po"¿ùë›oÉ@›-—
H@¤è¿òsпçÞтFÊG¿èÒ=؆¿áɆµwÓ¿å"DkÐï­UNASNone?ïÑҖß?sþ¤ãˆ%Ø?>ÃÙ¬"]?9%t.mš‰?u‰zF¤?sn‹²Pù°?ïPš¥ïN"?˜kĸðæ¡?tx{"¸8z?ƒÝÌ-#|l?ÎŒe_x?'(`MEú?íkuN¶œ_?š–·tÈjB?–ÿb½íD?29gB—õ?­Èúÿut?•ú`©š
?î,¼J[·?œ¡?ÌCœ?K"õ°(^?KüúËyT?¬Å냲¼?œiƒ7Ž{?ïñZ¹gÒ?_$Ð`Ãø?)H–*=uƒ?#íוü©ƒ?Z!zR{`?^Ù¸Þ¥]?ïÌåÄ?Š"?vÚÁci€?Yómg
÷è?^\1¯|'??sBoʓç?q»à^%<?ï&Bb-Ð%?~9…zXVÈ?'q'ÞLM¢?g5shN;V?'þêM³‰|?x‰DR?ï–^:6Ì_?vcïÃ:-?(é¿N½©?#Iîݺ?ŠÊpû5ƒ?v9vèðgAGN3FGL J1949.5-1454@9¶¹ä'¼0À3v…3±tÀ9´ÒŠ{ïeÀ;n"WBÜô?óZ¥óš@s¯H'zÄ@Ž@À9–z?ç=Û­»:¿åJÁI-gå¿ægò(b0¿ïÿωþœUNASNone?æOÁíÌ?ǔj>Ñæ¬?Ë÷
¸ë™l?ÅV¨á¿?·¯qÅóO?µÊ9"4…?Ö{#%¸»?Éb©©˜P€?ÛbyBD°?Ç[ў)›?Í04z*?ÁÓIh©·Ÿ?ÞÏ5žX¬P?¶»*ú¤i?Øír¯}?¶ºnwî(?À†•ÛÉêÅ?£úÑxRn?ÓÁëzëa?´ Bom‡?Þ¯Pxq‰?»D‡À‰—?ÌmÛ8(+?´û´Ë1Þ?ëûjq/d"?¼,øz³?µÝå³Âr}?·;^¤éö?¤…"ÑÆ?¨Ô±æ 4?ß`Ç·JjÃ?ɀCMBå?Ö\Ä"ü{³?Å
(º€¼J?ĄèKr3?¹°²Øãd?æÿš¼?±ê6Âß?Îû×|S7µ?¯Þ‡¢Zº?±‡hö€Óº?™&­M\}z?á‹t;ا?°#oŸ3Ý3?Õñ!¹@Ür?°³•Zçúr?»ßØ5iKý?¥¢ZoRMIXED3FGL J1949.6+2355@NXG¡A)¿ñ×Ê÷àvÎÀ9#ª¥æ¯À:€Ú†?à2»œ"àÖ@7í&ßgÚ@Z¶ 8Ò¿Ü·N´ ·
¿Ö³'|¼6¿ì"žZ@	Ó¿ß21k

UNASNone?·´$\Ç$n?¼§";Vê?ÍÇ5`VyV?Ì
þ"M²ï?嗮ˆvÝ?ϋÓÓ|>j?µ©ÕXLøJ?¿ž	ã% B?Ã÷ÿålŕ?¿-þLîèx?èLÅ[qôB?ŇVѨæ?×&Á«§µ?¶-£'›íj?Ƒ­DqI?®òÝ>ËG?ݐ®~X§?¶ö˜êÞ_æ?ËK«‰Ø?¼Þ©¡­?ĐH2ÚÙç?¾oªæPµ?ä	x±?Ã8—ûM­w?È©¶—?È$nFÛ?Á–-Dlý•?Å
3nà?å"JAdÔ?Îî‰Nâ€?ŔˆîP«?Ç*ˆýó"ê?ÍƝ?¹U'"eÔÐ?åój}CÄó?ÉÚO.4?äid®3O?´½+h:[?¼nŁ:8q?£x› ™ç?Ð…CKYE?±³$¬0Þ?ւ0¼‹a?½Í'æg2?º_(ÚiÃh?§L¼äOßâ?ás…㦥?¿T=É(cMIXED3FGL J1949.7-8109@s‹ohÜÀ=ãæÄŗÀ9ÁC
›ÉöÀ;m±|å-í?ä¢X —>@VŠ16"@šwàŒGL¿Î"tŸA×Ŀ飨Dhuñ¿Ø©Ý ¿ê®iÆ~eUNASNone?ᅪcwÀù?†‰Èhž?v+x6‡?…~Ar'Îâ?d¬T}Þ?d'ùâ?î§çwü³?¢+}5¤–g?‡oëC×Ü?…èýɳ¬"?ŸK‹£õƒž? Pží°6?í?Î "Îü?¡…ªà?¨ÉçÒ"&d?™"úÊì4ã?£96+°éà?'{Vý+©?ëê)ø?¨U+φ?"4mÁr?‹R÷TÒî?ÁYj³Ø5?¦ocïvl"?î¥:Ç­²?Æ!È7øÐó?¤•;ò°?ÅÁú´š.?aqy÷143?"ŠL¾'XÌ?ï}³ÅðÎ?Š&Bz?tæL§Ñ?n]»¶ÆH?†J›­æš¹?†´;-4?îƀýbä?"Dð[-‰a?š‡Nƒê²p?',ã?‰Q#©ÀgÁ?x§6ý ‰Y?îEP*©¡?‹,g
ÁŽÊ?'¤»‰¢2?vENš–?¢ØŸÑ²ˆÖ?†~ï".+AGN3FGL J1950.2+1215@IS6Þ¹^[ÀxK èBtÀ8Ù°i¿·;À;øìˆ3?õ…*ôö6©@Q¨ò'$\@à`}n¿ã
l"Y¿ç¨6©EšO¿í‰Îtäûº¿ïþfå^¶fUNASNone?×cîFÅb?Ç9vÉ/?ÙU¶:?Èñ³Z¤«	?Ό¶ýW¯?ï¢7«p?£-¾ï³dm?©kþ»8N?â…
©¯ÄÝ?ÞÓÑ_ó?ؐ2Îņ™?ÊBÙÄW?ܚÁ/pí?µÍH‡?ÓcîñԈ?³áPöP?ÐðOÞº‹?±—®–'˜3?ºì4éc'å?£ÈX7¾L?æ9¦â#î?¹DŽÝû^¶?ÊþïÅÜT?³=i•ï?á ¯ãª?LJÖkº–È?Ö!kù+@?Æ 
­xÚÃ?¾t×\6¦t?·a¹$·a?¹>ËÁÚ·c?·ÉKwu?⯬ês?¾Ø"?&?ÔR)µ}r>?½jf¿ìXr?嗭ž^Ol?±°Ëù˜s?È­w½%åÃ?ªAI/²‹?ÀóÑÉ`܏?¥F¥ðƒÏó?ÐÍÛÚJ¨Š?©"ÞöFÎ?ân·™Åõ~?±Â˜³?Ä©iäRØó?¤eVùb.MIXED3FGL J1951.3+6909@Y]uÍ·@4#ãŸw),À9÷Š1FÉéÀ;À´4O'å?Ôîhæ¦ñ@Òbœ­JQ@•ÀoF_¿éí$
Ú¿ëÒÑøß¿åْ 1+z¿Ý.ÚáÆUNASNone?ïÕ߂SyF?{má'Úñï?<šcƔ?BÏ9KaÞ©?sGEGµ†Â?zÄ	$ÛóW?ïVšÕ?]?žP±R°Ây?€ÃÄè^B?‡†Jj.?‰•…ÆzŽ—?—Ð#ÿ'?î",yI†Ë?'ù£x¥1?ŒúšQ'ú?yz9Ü_†â? ~¸¯0I?ŒÞ'4€Ã½?îHO¥Û?žO26@ÖJ?‡×A"'¯£?†Ñúð1çë?¨%ªºwak?šªãðŠ)*?ïóð±È(g?`…¡Ò'Ÿˆ?*Û'
•ÿ?3¨Œ´¡?TÃ<¼óü?_KôÃ1}±?ïÈÙ ã©?€Z<U~‰3?fy¢{¾?hi?Zó€?pVžÈܖ?xyA€Å	¤?ïiüÚä?xn‹é¼}?|là¯&ü?fwQOÒo?‡xÄUè'e?s@6¥¯…?ï›TÞîQF?zbÜYŒØ#?r>Eõ%†?d'·—| ?€¥Rûx?u!†ôAGN3FGL J1951.8-1102@=°É2
™FÀ2[Õº²À:Á!ßyÀ;eºßd?èr˜7]©@Ûï«ÉòÓ@֓À;ÄÒ?ï_»eàô;¿Üѳ¼©¿äÆ«¦j%¿Ûy%è"JóUNASNone?ï˓¶>?tpL{Q-?]ePˆvæ?_E]ˆ:?rÝ(uÑ#°?o«M';J?íf¦Q°CL?Áqêj¹Ôš?›ړ—?ªzŠ /w?¬-œTæµ?º¯Â¡‹ç'?í¹JP¨†i?—sÈ?œäEÒV«\?‹OÙ&åV?¥ù8p\Æ?,ÀŸµ?ä»L"'÷>?¸ð'Ùøj?¶®±ÐõÎ?±ÓƒÈ'y–?Ðݺ±Ó]q?¶³ýûœWµ?ïëÔã$Z±?^€Íɍ¯V?E~gá6ê?H~ܗÀ??]—3ÚÃE"?W"¶C½?ï‡zL>?­Ñ?ݗ?"f3	õ?'3Æþm
?•Â3çI?¥æÄîҞ-?ïA 3fµ?"U¢&戳?‹h¿B[ÖQ?|©Ms)Þ?ŽÆØ»Pq?v½E6	?ë‹&ÞÏ?¤-Ûáe?©RÙîž?™
­Rêûº?¶þJú'<?ŸŒMÂæ§AGN3FGL J1953.3+3847@RzAc
'@~¡ÆÀ9T†È½¯À;
»3GU)?êU7°×‰û@
ë×j@zoÜÝ¿ÜòD…ëçÅ¿çÜ%ìèdó¿èz0¶èE4¿ïÿ™àóUNASNone?ᆷ&M®?ÊFÃ{óÉï?Ã?¥bá²É?¿ºÕ^ì?ÓR¿T‹??ÈÛJ§?Æ~›´Hi?Áãcù4ðß?Ú¹.¥.ù?Å*Æö…>?ÚËäû?È%bÙ
•?àl&¦ ÕQ?¹#8=ñî"?Ê"Mz1I?¯ú3EÿH?ÑÆi
<¸?·/u,a?ÆÃÈoÅá?¨ªL#¬ô?ÞÄ:HÒ­?¶ãçgû?ÕÚ>ŠJc?²°¢¿_ù?å?L·qN?Èîûž¤ùÓ?ÁôKۏw?ÀRÞ§É;?ɁF«Nè?íÁ_Ân‹?ÜÌqo][?Ê"}'hg?Ò]Hk"½?¾/«K?:ö?ÐÖFÊ%
è?Ã_ŸšïÒ?灷ZtÀœ?±–Õ—g3m?Á®jæA¬·?¥º<àÉ3?ÀJ·¯ëPØ?¨4—Þ#N?×Þ2ÆÚM?«ÓmRxNÄ?Ø7
ž¦Ñ?®H™‰-?ÏÕÒ\%<G?¥g­Y2ŒMIXED3FGL J1953.4+7653@[LлnÖw@6ö¦ڜ™À:;[dRÀ;Èp0ꃗ¿Ð1¬¦ÍÅ×@¸1Hwh@ØÀ€
V¿å>ú߄µ\¿èUDÔxñ¿åCŸjþ&¿ÝÝ=ÄUNASNone?ïïÄÏZú*?[\©üv´@?G7k6õ'?HP?¨ßÛ?TÚÒë"*?T…jÊ%?ï•>—ÛÔ?Ž³èœñ?tíîtd?zƒ-ã8W3?€9¹d2¸?ˆ1 YGâ?îìBw/´?ˆÊÁJ[Æ?ˆï¤X³w?xmR1[?•ÿÞè›Cð?è"ŽÙJ×?ï&ۇ¶ÔN?‰}åµ±:;?aw'N–"k?_ Êm?˜õž¹ORµ?ˆ§±h4 ?ïû©züå2?;u1ó.s€?,Ì> ̄?-›|ʕ¨?4N
'¿ ?2¦§:iLé?ïÛ¾7Ô
?o zñ"@–?]ü½`#?W0?ÈøÃÕ?eCjnûä§?i7ëE27?ïŒ è¶jé?v'ù³Óá"?yñò®æ'?q°¡(ÊE©?ý™­jxÆ?gwå_'Öæ?ïØ¡ŸL‹õ?cI£MÓ?FbÌ®A°?7íTLð®(?pâÖâ?ô¹?aî^ÙÞdñAGN3FGL J1955.7-7019@tQ!–R½À>ÓKµáÀ:p‹¨?NÊÀ;̽M#Ÿ?Æì,­Nœ@
+Š•š±@
@/p¿ãã…³¼8¿Ød™ó‡¿â1|ÇX¿á£LúôAJUNASNone?ïÅ+y©?xÛÎŚ?=tMhîGó?8À{"‡J×?{™¥{Ï­?xF	.¾ã?î÷센×{?¡Ahݽt?(ømIºu?ƒ®b*Kë×?™81K†Ï?Ç¦bÎØö?î"iܒ"?"'$ç&Pˆ?"u¹ º¹?€&ýÛ£¨?¤¬ÜÔm/L?'P‰q ?í6¨¢dÞ?˜"ºÏ¢©³?Œ:÷'èú?ƒ!ÿšÜ?¯ýבäÓÜ?•¨q°‡J?ïî‰i˜?a9—«Î¿‡?,>#‰^?'.Çç÷6?`5'ëòŸÍ?`¥¼Æ"^?ï°lÉÕ]?ƒùÙ&
?e±Âþ?fã£?}?Ž…qH?€'g3ˆs"?ïQ;õ'+G?wáøö#òÉ?ñŸšÝ?iDãô®€˜?Š¥itÆ?pp׎0ק?ï\Ô|n?x¤tNëzT?xûã|ÅÛ?b²ZìÆÎl?ŒLï,?tüîb$·AGN3FGL J1957.9-0712@@ÿùÆ*\À2Ò^Ý)À9ÊØ>À;rȖg"¿Ð¼[\ê^%@
£prƒÖ@Åz¤6¿ã
e'ª6ö¿éÓb¾™¶Ó¿á"3©®BQ¿è‹Ãÿ/UNASNone?ìå^'ZÛÄ?´U^"¯?€Eܗñ?…˜PÇ­N
?¶ÒB¸¤[E?³Ub™¦zk?î¯ÿƒûš?³¼§'l?'ãyhtÿ?™Ç"Š|?¥³CV{Í?®!`cGA?ìJ,ÁK‡?¦sP‹†ý?¢	ÆÓ8¡²?Ž
d´"Ú‰?¶Ë/xs?¡¸D¸=_?ê)ËpÂ?¨æ¡xðg?‹ÝP‡š­?"ˆEyÕÜ?Śþ•ê
?¨$6_öPM?ï}ϛ€›é?')ã+Ȁ™?Z°â"9 ?`ZFñà?5üíûo?·p"õ?ïw†¡k?"õ,û&J™?s¬^ÖÃ2?wª‹"{?ˆf®à¨¡Ê?ìj£—1P?î÷Ÿ³±j=?…)››+³ñ?‡ß³/Ҝ?s¦]âÈ?•0:Ï?_柊Ô?î;췛.¼?Œ[W61?y҆Žé¬?cfë•ÆÃ?©㳓÷¶?Š¢I‡¼sAGN3FGL J1958.1+2436@O#´·,ÀQ½í@À9Õµ•x¢©À;[L
ÀÛ¡šÀ`@Ù2¹e¼È?úÜjŸ01v?æM"xºžC¿àƔR̚g¿³4ÊþҔž¿ÛPý~"xUNASNone?ïF•N—xé?¤8<'¾Ÿ\?UªW`d?U£L² z®?•Ò°¹K"?¤kI¹Ú?çkf2ƒ?՗¤3Gø_?";¶]¡P/?¡Çðãæ?ÏÊðkYâ—?Ԝ'yÐã?ìèÔU_áp?¥xZ™ÿ&?•à.·'?ƒëoVzb(?³qåG-k<?£X€©ñq?ïJ¬LµÌf?"ØV¶—E>âò·@?>ø4Œ¿æE?–¨Îé?"×SHvs?ï†IMPë«? \ȶMì?M˜"âŠ+S?SQí'zûy?Œ"$mPC? >ˆ	\?ìOh"Ø®q?ÌÛ¤àË)?ŠÔdñœ:?™ØL\Ïä¯?º*.½,Ƴ?ÊK<®ý:?îÌ©4:D?'°ÐɯØ?…Ùö­¦(å?wA'úW¤?›}â;Æk?êÄPɾ?ïÌÝ\x7/?r-#æðR¤>ÇwÿÔg>Òëгp;?yŽb¾šÉ?r,9XŒ=AGN3FGL J1958.1-0243@CЀ¶sÅÀ0>h›À9‹•¢"À;Vé<o?ÇÂyë1@
O^b@ìi_À¿à—%oŒ·¿êðò	áð¿è9/B[M¿ïÿ®7¥!§UNASNone?îQäáVÙ?¤¹ü¬â—Q?…5l†V"ä?‡
äöãld?¥"dlåQ@?¢(±]²B?绢§WÑ?ÇS}¼ª{û?¾¿—§snY?¶ŸÞ00ü?Á±¬!¨é?Àá¨#þ•z?軆¸Z=Ó?ª³u7åtŽ?½7ov
+?¡?‰Ö=?¼ìZÇ æU?¡
µ¢É?á.u³­¹Y?³ÛèÊÌoï?Ũ'=Cq3?°Ÿ±
as\?ÒÎËúÔµ?³H %?ï2f¨Oã?•‡&‹–1ì?yº‹óýo?~CØ2Î?"Dˆ{6=?'Á	M›9?ìן³±j=?¹8C3Ž?¦‰f€Ül?£Z%ž'?«üý_DfÀ?±žÈ¼‹¥Õ?엄RNp?? G›¸[?°À]ò‡C?–_<Àê©?¦z:"£‰?ãýqفÔ?éç9UJ?£8މ[á?±çᩒZí?˜ ÿàÊ5?¾ßìŠécÃ?ŸŸðÐò}AGN3FGL J1958.2-1413@;LŽÞT´À5§ÞÖºŒÀ9Õ¤9/ÌvÀ;t_˜?õ#¡Å¸@Ä
Ò¦€ˆ@Q%¿'6|¿ÀÈk%^¿ê!ÁduÍ¿íi=®ŒDò¿¨ÃG.ÇUNASNone?Ûà¨ùÖ<°?Ì-å>fJÀ?Õ®•µðxŠ?ÌѼˢÖ?ÌႠr•Ž?ÅÕ:D'è?ìÃNx«YØ?Æ8%–¤Ã?¤¤0W}î­?¸§h€-H?¯&è\×Ú?¼žïŒóÌt?åt×܆b?°¥™ËŽKl?œm²­^??©¥‡
¥Û?ę2Û8d9?¨m›ˆãè?áâÿú Âî?ÇX8-÷h?Ã!¸–kÅ?Ç~'nGÎ?Ò©#ËóDA?Òj»=?äƓŸ?ΎËÛò?ß?˒§—´??ǐ{÷È#?Äj>7«à?µP ÿª?îá],xPk?³
íþ¡[?Œº8S6;"?£uµ>Ô?•w>@{œä?¦á7ÿ#?ê÷ëgR?©
®âùV?»)"°{Ë?¢–Au>'?³ïðÛé®?ô"#ÿ\Ä?êg‹â̾_?·ë¦¿û`½?¶%öwEI?µ¥iŸjŽË?¶ªÍjùÀ?©"S]¹ÞLAGN3FGL J1958.6+3844@R™é9êÝY@hg~"Z•À9XÓÍ$áÀ:ﺽ֏Ä?ÚlƒÁH¾@ÉQàd)@PŸGƒ¿é×*'EÑ,¿èZAâÎkÞ¿åþ	WŽÿ"¿ì+€áUNASNone?îßã:!Žñ?¡/½C(/?ƒóêóÔN?"ƒUVëìo?›AžÂ´Á?ž¬dÀ_[?êµÒ䂺Ê?óíBc&ì?›™ÿ½\cÑ?~`}¼?ÁµtvIˆ_?Á›Þ‰Hú¬?èŠÌ5Å£?´/F<ðä>?²²¤Ëb? 2ÕGù"?Ä{}9f©?°ƒ†bÔ7Z?縔S$Š?³5…àvš3?¡8€g(	2?jø%Óêœ?Ìώ™Çx
?±Ý2Z%t?ïT&D&9i?¥æ¡"È?u}L_Ë?{%½BW÷?ähô?¤·'Ȳo?îc%ºW\ç?­ZÖéšÞŸ?†<eœ:?Š‰Î{°?¤>¢œ'?¨Ž×b–½?ìx{
Ùn?§9ås°Ó?¤Â^OdÃÙ?•Îh7´½°?±Úø"ø(?¡ò†}"¦s?ìj!® Å?›¦ŸêÖ?˜òú/œÕØ?~Âʸq\?¶r8¾5Ðß?˜ŒìÄMíAGN3FGL J2004.4+3338@Qªõs}¦?ò÷; ¿þˆÀ7Þ@c^JÀ:›ò¼K?óp"£¶S@WÉy[5±@^Ø_ýì¿àáÐûø¿æ]ª8*òP¿äË4àÝP¿åiÀBеUNASNone?ЦÑ;f?9ÌÝò?Ô6'<9'?ǯZX U?Û#ϝ·‹r?Éèá­{ñ
?³ÍVÏ3s?À'1t°ð½?ÍÐZ/Pð?ÁÏweÖã@?æïÉbEV?Æ)CJ|À?Ö¶,`ÊßÑ?¶¸Þ¹tÄ?ƈmÍ8¤?ªü2Æâý?Þœ¹¬?¶ø}Üåù¸?Æí5öº'?©ñW7v?Ï=Bô¤à¨?´(í4 n
?âuaÅ(#ò?³i؏7eÔ?â…xñ""‡?ÊU†T>?ÍJÄ¡|‰`?ÃÏtx^Ð?ȟW˜1(†?큪B<?Î+i<x¬?ÑI¥¨$½?ÎOÝvEà?Àx: H†?àá.>_iÑ?ÌÀ×gÉý?ã•`®…RÔ?´+y¢b¨Ý?ÁíÐ}†h?¥Â'V?ϼ¬ÈdL?°»²xĪ?Ô5ìEZu?¬ãN»Ç8?Ðòn­ÞÁ?§Óá_ž#¬?Ú،f³ÆÊ?«QÔa'MIXED3FGL J2005.7-8241@smÝ/Ÿ¾À=:úÖËSPÀ9ë:жfYÀ;‰$Ų&?Ï­¥EýÄ@ُöÏc@p0`E)¿ç"A¢¿é¶ÔÕ|@:¿â»|y(¿ïÿ­½Æ}0UNASNone?ïøÈ`¬h(?K¬¿´
Ո?!>š"?$1;ëuOÔ?H™­õv9?I㊼9<?î`žXùŸ?£?ùù­_Ý?‹4‰Y!Þ?ˆÿð|M?¡<Ö7>6›? C`Š«Ö?î·e‰"
[?Œ2ãvL]?"´¦s»d?'ìKE¸A?"^¨Äê15?ƒ-Sr?ìê"%ÍM?§O›5àh‰?—e°¸©?ŒJ•[ŽŸ?¹òUƒ¦No?¤´4õ\d?ïû©-­¯ž?;ÿ"Ùú\?Öµ§Î?PÜÅj«?<Aý«Aì?8¼BrÚÍî?ï€ÙCJ$?‰Ptؓ+?tB4‰Þ´?qgý»½:õ?…¨®#Š¾?"6DÈÏl°?ïI¦æøáÂ?|‰Û0ân?ŠÍ1e–?s¸N¬fH?'É#ÒéÚ?q]/XL»!?îÖ.ÖSè?†¹CՃ.è?…­Ø¡ßfÂ?n¶)\™­Á?šc8í. ?ƒ¹&䅥AGN3FGL J2006.5-0939@@Q'>EÀ5‹&9O­À:˜._ŽÜÀ;¥1}PŽ?ï™ÿ¤ª2³@õæÌ}G@~Ûÿo·H¿ÜBÈÍ
åF¿éC¥×?—p¿ïþOÃ%ã?ïͦ¦óIcUNASNone?îÇÐ#Ìì`?¬7)_ed`?´">ÀÆ^?ÚJð±[í?–QÙN€åš?£DÇ4{j?îö£T¥Á?±V;e7»y?ƒD'2r?ž>,*qu?—‰U¤ƒIÏ?§:Wf?ê+ÍÕ±?§Þv•Ïß?³1M'ç;é?œ£äÔ³ÿ?»pIáläQ?¡u0»µ?í}}F|¼?¶aµ)¿'g?‡+¼Ò\B?¥y¤1¨7¥?±.²ÕÉ®\?³»ð¤ çI?ï`(#,!h?­…!,>…?{‰ àSG?›öãá6GW?Š1fӔTE?¢äÒgùª?什™?™s½Ye?oæh'
?Œç)ð>kö?|.C6÷Ï?‰;NúRÜ?í‰þËÄÜ`?™ñ²®?¡¢®â?Žédê¿\?¥½e3ˆ?'lÜ;ž¡?ï«»lý¸?£@çoÉ
?`…rFù¡ˆ?ƒ'¼ŽÈ?€ï¿_`Á–?ˆÐâ^™
dAGN3FGL J2006.6+0150@E¸²•éá±À/aǛ4¤À:3ùJYQÀ;›zé¯?ðÝ ,e@:%Ïrn‡?ýô€kJQ¿ãÉÁb"ü?ïÍØWiJ¿á`pX
a¿çµ>LòUNASNone?íœqCÓÙ?´®Èú·?–f•À"«?žûöhÏÈ?«
Þ	Èò?°^œðB?¾59Íö¡?Áy\LÜýr?åE=€•"?ljgŒõ?ËÐlÁ–°(?†™.18?éõ]`iˆk?²-	iqné?³z±p˦? Î°E»G«?¼ÚúLŒË€?«žþlçÏ?É@¡t?ºýÃû`g?èµÿÖºa?À‰"£"C?©Ä‡¿2¢˜?§ñz
›?îô¬‹tùã?¥ò+?…ûK´t·?‹aNwÒâ?–lÉ­ó5?ŸãÆæ
MŒ?֖ÏùÁ¹?Ëv§&J¥?ÞŽ£"ºÕ?ÉýïžLË?ƛBÄ©Eg?ºÕ+ÅD‡?íˆJF "u?ŸûËÉßµò?¢ÊҾ׫H?'‹"];R8?¤°ˆÙ¹âh?"ç¹ËìE?ß±êXxçó?º_{™1?ÝÀX™¸è?ºÉ~›ˆÔr?¤mèttÑK?™mo¤e–MIXED3FGL J2009.2-1458@;³íÇïzÀ7Ôé8yÄÀ9¢eYöì[À;d¸€åm®?ñK×+Ë_å@i›ô<ÓE@' ¦Ô¿å|!SŒÄõ¿ë¹©#Ð>Ç¿éŠp|h¿î¨#§Ù›UNASNone?ßvŽ×ôž"?ÊÌ£ØÈê¦?Î&VûS6Î?ÅZ¾rA?ÑvEªaÆw?ÉjÜü«ô?Ò6g… =x?Çl»ŠZ6'?ÞNô{"Ç;?Èw›¸,פ?ÎõGþyöš?Á©@²£?ã݊s¥­é?±Ò"½rÙë?Ìcø\ˆc?­4ȈÀ9‰?Ä%ÝÕ]¿ú?¥ŸÖ²oL–?Ƶ¸ÔGjx?¯ªŒ0ïD?á+
ZÕl6?¿GٝëØ?ÒOà1rX?·÷U`w?á°_üv?ȝápÍ?Ðå .oeO?Å7(ö™Nñ?ÉÙþ#1Š?f¯?â]剏¾Ø?ÈâÏSËë?Ò&х™?ÃSƒÔF¥?ÂdÊùn?¹~†…Ð?é¶ôY"Ø?ªg‹™Ì{?ÁÂùAþZÂ?¤'ßýß?³´UÜ8L8?™ñI¦3¨E?Ø 
¬eú?°Q–u¢Ä?Ýj•Âkí?³ou/ŒH?Ž{¯4?¦0yY-#íMIXED3FGL J2010.0-2120@5Fw_²íþÀ:f	EùßUÀ:.P‹2ΉÀ;¤#ìnS?ñŠ¢`<«­@
[ûÈ7ç£@l€xá=?ïü[J ¿¹i8þ6AÕ¿àÊÂè-·"¿ì¿.Äí
UNASNone?Øf
7  ?ʍÁÌ5µ?á^—ßýx‰?˜†Ç7• ?³s£7¹;?°X9,:~S?Ð-IÆêQ?ŌóvX¡?à=¤ÙÇ9Ã?Ér¾¡Äi?ήÙ
·'Ò?ÁÊ÷î'?ڍT$£?·{æ%²mÛ?Û±©Gƒï†?¸#ŸO?–ȮÚô?¬/CÃ?Ò!Ll{dŒ?¸âÃF¸·q?â/ŽnJéç?ÀO¥š-é?Âÿ-mݏN?²$kN•€?ٮ˜óü?Êj¯cÒ°?àḗ¿,"?ÊÕÌkº†?²70â@¿r?¬éCNT?ÝXŸ|©?Æ/:¬h?Ø+¾.h?Äâg'‰÷T?Äø‡×‹}Þ?·	'\ÌO?ãnbÙ¢Q?²"d—j{…?Ó0fou®®?°€F9Ó5?·ËV;\2Â?¢'ã"wa?áíŽÒÀ'?²¦·´«¦‰?Öâ{M†Ï?²ìÑÍX1?µ	¢4˜š?¢fñJ·\™MIXED3FGL J2011.1+4203@SŸ …±…I@_î} ½À9?Ú{9À:ÈTà,%"?õa
1@ë@
²ká$ž@I« §U¿æŽXõÜÝÞ¿ê÷å#¿æøá–ïi¿ÝÃëfjUNASNone?ÒCò vöŠ?Ë
#F£tÜ?±C_27@?±\0{Ÿ'ë?䵛	}¤"?Í°]Þ1­?ç}Üz?Ðl¼È.É?®RŸ
üñ?´ÃÃ~""?Ȭá·EQ?Ê&ò›qÅ?áŒÄ/V?µÖ[ð*oÌ?Å,47%l\?©°îÃPð?ÓK¨Êäë'?³ð]I?ՓEšMô?Á[E×#?ÂPUýQhÂ?Á>¯=DÙú?à¢Gý^~Õ?ÂъûàÐT?ÙsÐè÷a?Îdlªçäo?­"@Ü`Šý?®-"}À¯?álã}¾FÍ?Ϻ'$ÄÊ9?ìßӁûK?ßO?ž);û":®?«¾å•†ê‰?±}Šb啀?ºÁ"]ÀO'?çÄ_WWÏ?¯qJùÅ?»y÷Š2ò?¡ûªC«"|?Ã1†à¯WÇ?©0O7§Ši?àf'¤Ä\?¼^Iùj²?È«L"®"h?¹"‡dkm?ÒÝ4l î?¹¨¼Y.'ÛMIXED3FGL J2014.5+5246@Uøígwž@#Ìó˜éprÀ:3o­7PÀ;k¹Ù&w?íRŒ#†º;@#¶XzÀ@bÿèƒ¿éõ'–âd¿ïÿžæWê?ïúu7B?¿Üº ÆUNASNone?îÍöš'ˆ?¶®|d0o?`cè'>ïä?g¥lˆÙËÀ?¢WÙ«Ž?¶œ"›n?î	Š#@20?¿Ó›!rÛ.?‡
âÏF
{?š¤ºK8?©¤¥+Y›?¼°é
íuÜ?ì[â+%?!?¤Ù±:3ÓM?ôàv©¨Ñ?šXÎ{¸-?µ£¶ŠãjÀ?¢^"{uÖÂ?îbE—¹Å‰?¶OÛ? _?a4Œ')àZ?"¡jɘ'?¨È]ÂÌðh?µô¿6î?æ+æð†Ý¢?Û'ã_qÍ?Pĸ*¥,a?e–Ø\j""?ӗmfØ°?Û0BŠ`Ž?ïZTƒ
?®à풫mö?uÿñiȜ?æMý8ûI?ŽùëÀ¿>?©¡Zì¸*?í«Q/¦? Ü±_G´?‹Píˆxå?n®B#K?­‹Ã€
? NK]8¤¾?ï¢zŸ"–Œ?˜8oÄDNJ?k""2Á\?ˆ4M='ä?€|'N.$Ã?'8³G7'AGN3FGL J2015.3-1431@<ÎdÜY2À9oç¨mÀ:­{έxÀ;µ}Ëùï?ÊÈ­Ì_N@úٝj´?üSQ@g<?Æ]E¶©•?Èk"…þŠ¿Þ{V¦-¿ 2
W!<UNASNone?ï×Y¨&?o̺†-?Gà:ÃR?Ec>¤7¥±?qoÙ£h. ?muAn?ï;T5Ñ?žXó§¦?v U'†
v?HB`Žl?"
cډ½?š](`W"Î?î'Cñ–¨?‹±Ó B?ÄaöÑ>?{fxÍv¶Û?žó€:®ïÆ?…%±FÙ?îEŒ²ç"š?ó›ŠãÝÛ?}|^
âÏ?ƒ5ävý?§÷²!Òm?œj93ò-¬?ïò&oø­É?SÀÛ"3/O?1¡±¬?.z÷»¦ä?Wl÷‡…ú¼?R›ÉQœ›?ïÃ)Lv2?}¤äA?^Þº,ƒŽ?a휯²by?v³«oƒ;K?yˆº{Gé3?ï[5/Y+b?v<?kÑï?€·êÆg—ç?hÈúÓ@êa?ˆzÉYV±³?pâpÅl?ï–þJY{®?xù	ü¹µ?d.]_{k~?^¹³(ڔ_?…4Ö
3É?vsZ*nïœAGN3FGL J2018.6+4213@SÙÆ*\}@>"ՔÀ8wöº «À:€
è j?ñŽÑä›@¨RÙÛ_@&«ÿÍ«¿Í¡Bt2œ¿ëAlKO+.¿ÜáÑÁŠú¿ì
2ŽÈìUNASNone?'[ԗ:|z?˜¾¦	ÅÀ?ËÒJ<[W?ɲB	1Ny?èxŽÌX€?ÊÑ^¬ÞšÖ?¶}
DÎýY?º^+d¨?ÛZôD']_?ÄwJ¸´?ßÉ)÷l«?Ç=Á2 ë?ÆÁ°"J?­Ì*8ÙR|?Ô÷<?©ì¬?µOw5¼[ƒ?ߧëv±R?·'J\ù‰?¶YPß2Ù?¦P^Óz.þ?Ëýjà"˽?¹Bý«L?æ5]§iÖ?½äNkm?©Ë嘶õ¿?±.ÃëZ?όpH3í»?É1?]cŒ?æ€%"ºÕ?Ìg?îò*n?Ì ËåÏ°µ?Æ󎠟ÐÉ?ÚªÃmR"Ì?Àɟ»ò‰ö?×Ö Øt˜?ÃT4¤f@?ÚÉ­;?¥?³çA¶¤Yv?јâŠ#Y÷?°·H壽?ÔISÉ´G#?³O½ñQaS?Á0á©þ–ž?¯FÙrìir?Ô+Áá%8?°Uvôh?áø´Ç¼?·fÿ©ÉMIXED3FGL J2022.2-7220@t%VÿÁßÀ@LOô4ãÀ:¨t"ÅÀ<ÖÝÇÆÔ?ñ®hk#d‰@
>§3á?ÿ0Ñ@úÇ?䶄OÊ1?Á¿œS™k]?Ö(f")_l¿ìÞß}Ú UNASNone?ß8IIÂc4?͟¢),–ƒ?ܗ…?W?ÌàvUzc|?°ÀÅÞj/Ô?°6'¯í?ל=jf·?ÔuÑ>‡¶S?ÛK":	³?Ò±CG–m?Ê1@·!·,?ÁÜã·0>?ÝDà@_½?¶Üv²?ÙòVlü¶?¶qЏù?Á'Ó!G?§Ìk"Ï`?éH—Û?ÆØòËCœ?Â{Ÿ—?Åâ‰Jt ï?²æ[»{?²H)V¾è.?ÚéΊçúü?ÌÞÐ^Áp<?àòԍ$Z?ÌG[5}1Ñ?´/0däÁ?³8E'z¸ñ?ÙO"9Ç2?ÖЉ
bó?ÞAaoí´à?ԝ‰ÇÙ6×?Àß0±Û?¸à!N•v?ãºÓöIX?±n0zÀ<P?Ó.ZÂ}?¯' WÍ-?µoõFU´C? 'f!²¸?ë±I¸t"ì?¶KÆø®o?¾ N;ï'?µ{5{"È?'VS¬wE?ROd3ŠMIXED3FGL J2024.6+0309@Gzš€If{À3%oü^À9ûUê`oÀ;€.ÓR"?ëhSÃ÷f(@"ŠÝ"T?þŸ`A^D?âa6FÒ¿Ó}Ìyjп×ÛÞéëý¦¿ì¦˜	UNASNone?éo-9Éû6?Ãò‹¼ûã*?ÈƸÓh?ÃjäÐN·s?‡Ô5òŒAE?‡Ÿ¯ëèi?è‹GË?ċq)?¾ÿÄhF²¹?¹Dïíb?Àmñƽz[?¼-àÁ~î?äËhTŽ]â?´¨=Úسs?ЛP¶ÚOË?²¤½«Ë?·7z'I">?££›ý¬Q?åz™"BÃ?¶nu'dÓý?®áqóì?±Øîk0:?Çf¸M?°bœú¹N?éãÝY%Ïâ?Ãõêl3Ê?ÆÍŸ[8?Âa¶ScªI?Š6¿¶?‰œ:½þï-?ìt‹­²ƒ?´9®8-?«Û¸Êw¸?¤)ÓOR5?¬ÛŒYõQÂ?ªŸg/Pa?ç&ì©i£æ?¯, ¨ô¯?˚>/:«"?«™éáÀ?¯(<­Vü?Âù"tú?êç±"_É?¡:N5c?¸«#	
~?›:?U¦0É?°ªÈâyµ¸?–`AC,«AGN3FGL J2024.8-2331@4=Ž§ÎÃÀ>\ÜY1ÊÀ:'ý«'é¢À;̝{¦iŒ?é;H›¹|@
ßþWß:?ÿ2¼À»Ÿ?ïø̵O؅?ÚQY1¨!¿ÑçD6"¿ëŒÇÓá
"UNASNone?ï409¿Ðv?–úÅ#MFŒ?•ž"ú²·n?•‹K0wd?nÞ®j™Î^?l¢7r?Üm½Øñ§?͟6©+Õ=?ÖN-¬ØÞ?ʵ£"âá•?Ëd(ôjö?ÀRìYŽ"?ë8±ø50?¨Á0•iÌ?»°ø¬ŠÉ-?¤úÕâ‰ÈL?¨zƒƒ—¥?•†°×Ðk?â›éîÐ;?Ɯq;!?Ôȯ.´Ñâ?ě'GB‰½?·ýóÑTŽ%?¯×‹^՗?ïvâÆß"?Žy1DEª?ŠýE·Ïx?ŠZ0\›	Ò?mü¨OœwÔ?k›Álê_•?ãþй|Ÿ?ÊR曙¾?Ïç]«Æ†¦?ÅHøYQ?À_nFüá?³>-žZé?ìfÊwªS?¥5ƒß6ö{?µÉ8§=%?£/"cÁôÁ?œ=‰e?wðíârÜ?ê6ò…n?®èbÊÁ?Âý"{¼<?«í}ðry?¢8ëLVÕ?—‹oºwAGN3FGL J2025.1-2858@,Y'fw-^À@"Ý—ö+À:TŠBäÀ;°®Xm_?ÒÓ¥ˆT½@ñ8Hñ¶@}ûŸž¿è…¶ˆ×n¿äÍD¢úÊ¿Ü?Géxª¿ÕvØiþ»UNASNone?ïèØ-Ä?dOò Õ1?-w±áàå"?(?`Yœþ?f'¬'ÍÙ ?c£e®àE?ï%Q=ŠO$? /n\Èæ‹?xÕzåá00?…æ—u¾ML?• y™µMs?™Ç0RÆ?îZedä[?T;bùì¸?ïk	æ?x¹E&ìÑ?¢]ꮌ?‰ªÿ@¿??í!Ôç8^?¡£n¤€?}?Ñź­?ƒ¤ÝýÇ ?µbM%me? wȱ±©¶?ïö^I?Ê?JÎpvIJ>?"¼l\M.&?¢íÃ¦[?PëßîÜÑÜ?H»	œ se?ïºl'ÐQ½?…èqáN»?cª¼b
?rÎÙ!Ýàò?y;5Ó¦üž?|ù®d§S|?ïa×)¶Ìt?s50ëݗ¡?}e!4ˆ"?bڅ‰Ïœ•?‰'ö³Þ¼?j÷ݘá0²?ïFØ0z"'?€€KÍ-yÇ?sHéú?W?iI>#Ýmï?'_'¹Ê"ù?|¥•Fé3AGN3FGL J2026.3+1430@L¡WÞ
fñÀ*àÔº××ÃÀ9΃&À;˜(ßó?çN	÷^@ËoT¡˜@E¨@P}¿Ê/àýJ1ì¿än¸oüõ¿×û'hZK¿íi$;!GUNASNone?íéD©†?®ävUª~?¬ðHQþO|?­¸I¬ù*?ýZ[-´¬?}K"Ÿ¡Å\?èqT3¼y?ß̅÷rµ?¼½¯:?Â?´×¡YYø?Á‹rUn,À?¼!öä'*(?èÄ
ý´÷?¯Gi=›+?ÅúX~ÏÇ?ª†?kBÃ?¯¢E땼u?™ Ý<¨õ$?詸?nwN?°®?…ž\n?µ"éü9u7?§gîj›?*sB©?¨…µ6-8?îÌÒ硗ó?¨û¾°]? ?7¥îž?¦K:Ñ´©?wœÎÿÃI_?vet{`t?ì7û'P?µAõê?­¼ú'ì?¥×çû)ì?¯pcWw¼ù?ªXd@Øs…?ëvf%ÎÇ?§uW¢¬§c?»ŒÊ¤åŽK?£·.Ìcs×?¡…ôPh[?'¡Øð)?ìÍ©ixó?—C˜K…?®}|ÓFUÓ?'‡àApN!?¤§ì˜š@?Œ³pyG'AGN3FGL J2026.4+4709@U-Œ*EN@ÓáF×UÀ9rÀdß}©À:ùbLLà¿å|°R
 @ù|ÙŒ@|Þ 3玿â,»ç‹Y¿åƒ‹Ç·}¿í87V¯¿ '÷Ö:ߥUNASNone?æ|!ÓS>?ѴἩ?"•¡3`?'¸Æԑòn?җ­¤F#ƒ?Ñ"á‡Öò?íÃ;^Oì|?·¬,#"?	ø¯!>?¢àlm?¯ŠÙ§Ìn?¶^†'—s?èÀ ;Ÿ=r?²Çho65õ?±ÓU°";?Ÿ}Šó£ 7?ÄwfªÀ?®¼|yv".?ìÌÏEÆ?®Ä{ùÙFï?XE¬ŒWh$?dp†%¢"©?¹8q+SzW?®¯0Ԑ
õ?ézѧ?Ò!Eîú?žÙWFNH?"•xS¥y?ÈúÎ)"…?ÑóàcÛ
?ït˜qŒ›k?˜æbHÎ?f'L]íB?p*cˆÄs?9P€6vS?–ê‡ÙäÉ?í=ÎJ©O? toÅ^@?\ROþÑõ?Žú;?Ì=?­tõåé·?š)3ÇÓ?ï&ÿöÅě?‹¸Ñ†¬?2ؼŸêm??0;ÚÜÞ¹?šÔž:Xºƒ?‹{@ïòóAGN3FGL J2028.5+4040c@SËà"&þ?ò[·¶»À8ÑhÉíõ<À:O¶1ÔÌ?ôù`[µ]o@š
Wǽ@р:ÍÜ¿ÒÅÈ*j{Ž¿á†qŌ‰¿ë_=ú"¿ä~÷õ·UNASNone4?œÅe» Éq?¦U"9»ì?ÑQf.Þé?͒àG?æq!ºS½0?ÎçÝݞ߲?ÆþüƒžI?ˇ7Ô½Ì?ÂxÖ¢ÛÙý?¼/M~¸,?å¢Pž±?Ë$ÇéáF?ƍ€ŠîŸÊ?­èZkã&K?ÆtO¿þ)³?­ï'@wïo?俋íDÍ¡?µ"{^7qE?Âà3(mÔ¼?¶Ðc}zj"?È´¦c45o?½ÿ 3¼šû?åɝ íÔ?Á]'ð#z?¬[—zanP?¹À&KCJX?Ǹ¾1hì?ÉyU™ÜØ?èLü=J0?Ïdeüo?Ú>¹$_–û?Óe|w
Â?Àœ¯ÒÚǦ?»~Ò-¹)?Ýrîò32?Ðdÿ!øg?ÓYPٌM×?´ÒüÓlýn?Ä­Ž1ö6?¨¾2t)D2?áRì06Ëæ?¶ZÅᰐ?Ëž—°5g?¸"Þ?̈izþ¬?³Ë`å=Éõ?âþõ2û?½@ޖñOTHER3FGL J2028.7+1012@JëÍþûôÀ0Cý?[_¢À:ˆabñgÀ;vJt˜XQÀÎރ®uÊ@ËFºÏt@ ¨?ϣ¿èº"Ÿ"€Å¿èÀží°6¿åâ'ó~¬¿Û†u¾%ȚUNASNone?ïÅéòA?zoï‰â­º?R]_ÊD?S¿@'"y=?xâÇmaâ.?yHMò‡‹?ï |¬pXO?¥§X¿¡Ð|?~ŒŸ]k_?"7ÚÎw?"MBœëZB?œË'¡¨³r?ì֋"ČH? 
§ |é‰? ºÒD(?Œ‹óňU'?±CÉü"°?™Ž0–"j?íÍVˆU'?¦áX­½©I?9[
¨º*d?B"žC©£?±{𰧉9?¦ÓÞ¢­×y?ïèp9×oÇ?iÀ­0܋?@UÄ*y?EŸ''üNã?czz
×x?gX´Ål¢À?ï«úLëI?…ò»öp?`çÿ.ÿò?rZŠ1<?v6 ^­Õ?{·þŠ8@w?îÞ,:ñm–?‡‡OwÞõ?Œß{L½Íõ?{…êQW?•Êºý+4B?€f­qZeÈ?ïzñòºáØ?'!ybǔa?a®MC?
XïXQ	H?'ºtˆý?'À;°äAGN3FGL J2029.5-4232@ve†á›ëÀA¾^9q;À9Ö-Š|Æ$À;±+hc–¨?îsÛïÕe@
|+Þ«¢@öã•Ò¿åæɕµ´W¿äd"p 4º¿ídÓÈÙ<¿ïþ†ìwUNASNone?Ü|4r½%ª?˨;ydA?ÔBÌðÖcÇ?Çaûí§,?΁ý8Øí?Æy¦՞?Ô¿'ØQ‡©?Æ5:Á¿Iú?Ùêɔ€w?ȗŸR"öä?ÑU¤".Õ?Àt¸r¼yÝ?äøYŽDY?´"C:q¨Õ?ÉG?Ž>?°fŸi?ÂׇC‰JJ?§ƒ}TgÖì?Ñ4lJÎQÕ?´tÔ-uK_?â£#!(â?½»@¯óŒ?Ã
šã››Q?°èlŸUJ?ã
Ƹ¾?Οu#¡"ƒ?Ï#'!'Ô?Ŭ¡5f¶?Ä¥À«2?Â2²qE¬?âÛÒ"Ärƒ?Åj)Ku@Á?Ð÷§ýŠ…?ÂÄvgƒ¬?¢$ó ì?³¦`?Ýoð?êÞ6¢uÙ?§3I''Œ?¹rƒ+‹LŽ?¡56ó¦
?¯:†C
ŒT?––4ÐKš?ãTª;Ó?Ù?°osÇ¡4†?ÔgäòÇÞ?°_Vá§ê?³»Zº¯Á?vœí˚ÕMIXED3FGL J2030.5-1439@>Mã†Lµ»À<nš€If{À:¨ÂD³Ž7À;ÕäbÈ¿×Ûâ"Då@
h³'Š2ž?ý×>Ý
ˆ¿´SÅ)Åj¿Íºòºr,B¿àÒ­›rüf¿ØZg!ËËUNASNone?ïÓ& <(?q¨ì£!?A†µ`÷–7?;=ô߉á?t;ÙVgO£?q5"W!?ïdL_D?'óQÓJ?pôj{l˜?uÏá†Åí?Žr²ü¡c®?Èॕ?î'wtçı?‹%¾­A›?"C4°"?|qBwÇ>?ÎVŠ‡J?ƒÌe>lþ?ïÞYçýÖ?ŠH~°u³?]kæÍ8áS?Y¦e'ÚF"?œ-vP\=?‰|¡±Ù?ïï_,úù ?ZiKgÄ?/RÝ y?'|ßõ)k?]Wc!ar?Xí—à–_&?ïÎhÙ»Ñ0?s ÒÃ?Xù{š=Íþ?TµóçÓ÷?r4,i¬Í?p'ƒ€ø•Ø?ï_fÄ?x¼+é®?.ÙÍ]`Ä?pºpÊÍT?†÷ Œ²=p?oÖÊO5œ–?ï̧t½[?eC²Gì?EJBµ–
Ó?5 ¡®©?wý`‹?d:ë="}AGN3FGL J2033.3+4348c@TœŒ" Ú@Ü@Þ¡À9Ý©"â À:aþ£®$?çbŽÀwª@
c¤&œ@ð»`å5?ï÷Ž›Ðù¿ë¬Î
 ©¿áÀø´îc¿ãmϟ™UNASNone8?ÆëMîlÒ?ÇL6(Iå?™ŽûÌbÆS?žígšü˜?éx´¥Ê»Œ?È{ÃVÀ®?ÕáË淞V?ÕÏàž2R?¶xÔr`‹?¶ùÐú¤Žz?â?ÿ‰ãn$?ÔWOy²?û?ÓþàâèÃ?µ"".7Ï9?µ§‰› *?¡½h¨KhR?ãKžÊJ?·˜¡Sb­¾?ËÇ(â¼?¼ZPOðû?¤Ø"Kœp?¡•®DÏÒa?çñL­Të?¾Ê=ëëà?ÖIV­ƒ?Ðê°MRX?•Wîä~ä?˜Ò‡Kä/?äQÁtÀ—?Ñ%ÆM¤?áãÄb<'Š?ÖÌêm¶U¬?³píü¥á?´b
2ºß²?×\;¼æó?Ô#©ñ^/>?àøöº·±?¹juË8l?±ß¾ú5ƒ?žü{c0y?ٖ"Ì]¼?¸Á.ö"ùq?Ôð­¥rÉT?¾(­;j—×?±"m¾´.? t	'# ?ãU;uæA?¿¨Ã,÷MIXED3FGL J2034.6-4202@vq9C¬ÅÀB0øµˆãiÀ:~L69xÀ;©Ù¿#–Þ?æ!;xjä"@
éåµüÑ¢?ÿ+žÔA
?íåÐ6c¿B¿ç&çEsý?¦®o§sE¿é"ªß½sUNASNone?ï¡o]ù?†ãt\‡æ?cWP2ð0?g¬'µ)ƒ¹?'÷Îoò{½?ƒ^´Ôm?ì¿«)öä?³–Xn'¾?¡ÐtSb&?£ÒAk˜?±l…ÕO?ªµþÇI>Þ?ís%Âdò|? Bö=Â)ò?¢­ kUE?–
æý¸m"?¦ "¶±Î?'¹j4ö-¤?隊Þspï?¹öjP¼í?Ÿu2º'ß?£AÀV×.#?ŧ"mË?·ûWšË¼º?ïفž{*Ä?o›€WúD?Q¡S­í/¹?P»òà3é0?m­·ï×$%?iî01¶?íïB³XÝg?°€‹þøÚ?ŸjRß>ø
?¥dÃA?¡V«Yߑ?vGêVHØ?îÊöð{—j?'ßYŭĀ?"Æžº‰¶õ?Œ«èeTyœ?'Úƒ2"¿Õ?"[ÝiÂ<?흡´žû? ÂˆäF¾?ŸÂ¬X%?†?'œsC!E?¦D˜Z[>‹?˜_'
(øÈAGN3FGL J2035.6+3146@R5ËÿGs\À(IёXÀ9‡â3f^ÚÀ;Šyk%é?êTÕ£@…lP‹2Ï@fs€€C¿ë&FÌ'5¿ç¿¯æÀœp¿Ö50•ì]X¿æÓq†wuOUNASNone?îÛD«-–?£JNÐ!m?mR׌p­?n_ód¡ú@? v'OõÀõ?¢Žu±Ún{?çàã	¥V?Ì!náEe÷?¥÷¯ºÈ\]?§Ò@'âÞA?Êþ‡éݘ'?È®N'4JŠ?ëb;b<ò5?ª
Ó%¢?§ÓrÉÅ2?—³š$B¥M?¹_»4³‹¿?£W/÷öcx?è-$^a½¾?¸×WЂ(?‹ÇE.?…¨…lQg?͛"žÅ?¸US…Ã`Ù?ï‡Éʱ6?Žt2½þ?`Úóꨂ?bˆÅ¶Øï›?‰ÖЗî¯Ý?‹/•Ùkwº?íR¡ö4z0?ºÄ»›Ìúš?'³1_n½?—ÉÁÉqJ0?°þ#÷tùÏ?¶
ú!G7?îzÚÓºk?"ÙGð´§u?':$"¥ð‹?"
'"ã?žji|9o?Œ?Îßè²?ìÍ°:MŒX?¢Yç	÷?Š8M,TP?tô–ˆI½r?¶Kt‡6K´?¡\Ëäï/AGN3FGL J2035.8+4902@U­'#'@#M~8DÀ9Î.\3Ý}À;¨—š¼¿ê¢ä4â$@T(1ÍWŒ@Ãf?úìƿ䍙/*SÕ¿Î4Ÿ䦑¿æ¤
™¬Ë¿àˆàéiUNASNone?î÷u¬Ìɔ?ž®aEí?jö‰aИ÷?gıN"Ûç?²y9|Î]?ÍÔ¹Ên?í'Å"k©¿?¸*xíó%6?ƒ°Ehy?‹
!*æì/?°óʱ	dè?¶;¶+Îút?ì¹t
™­?¤Np…¶ÿ)?¢&Záçªã?'R'-›lù?±!1ßé7¦?ŸxC',ì%?ì͚'¼?§®•á?m´_ªç?j±[§MÇ?¸¥‹Äö'å?§kÏ°fl?來üI‰ƒ?'àC"á'?QݕýÙ¥?T
Êz®c(?"˜Î"Æ?'`¯Šu#?ïXìp+6:?›B"èe7E?k´úT6¼i?p˜Ožw?'kÒ¶ñ™5?˜':§QÛB?îÇ]2±Ð?Ô³Qú¿;?Î!ëËF?'ÂIFá?–F=¥Gº¹?…¼Ê{WÇå?îæö¥¼p?ˆ`á?–0?Qo¯	 A?C.Vüæé?¡ó@@þ?ˆ	Ä'vagAGN3FGL J2036.8+4234c@ThÕ¥¹c?ïèV`^åiÀ8§1"ÉÿÀ:3\m¿ <?õ"åm,©+@
êÇ+£ù@"€U$ö¿Åˆk><{±¿é={Êaô£¿æ'˦þ'¿ç
Yûsÿ+UNASNone9?a<_@/Û?`†Os³f?¦?+½\½&?¯.€ä˜¦?îŠÑ2ô/N?¯‰¿3҈?·¹‹qJ¶?Ä3+æã¤U?Æ:ýÏEš?¿
Ï݉™­?ç"ÿҙщ?ÈW)v_ǀ?ÁÊJ?§7Œ/	5?Ã&I¨?«‹NùA¨?æîú(Ïh?±íÜ+@sÙ?ºdfJ?±&WaùŠ¿?ÂYÑC*?¶¶["ø?è&ÿ1½¬?¼Ï›*µ­™?^ƒÁ€?js•ñ'Ø¡?¡È¬{¥f!?ªÚZÀØë?îÔ3·£«ý?«T"­økú?ƾOíKH?ÌÝÌÞYUö?ÈÃ6öâ?½ "•Àéa?äžFã¥h?Ëõ
¯E?̽«¯ú6Æ?¯ÞâãŠ_‡?æ%÷"þX?¨ðbjb²B?ãç–r¹?³9d馲?Á:o–ÕˆÍ?³£C¯ܱ?Ï-Úl%JÆ?´ª.$F*?ãåíÊ»{?¼PÔÕk.OTHER3FGL J2037.4+4132c@T7™E¶Ãv?ÒÙUÜ«g!À8˜-¹éÀ:2ÿâ£Î§?ê	ÑÇÞQ@
®¸–^ü@lÁÅm2?Âí'f²wÈ¿èôöЖ¿äM{‡F ¿äoñÆg"UNASNone ?t4_tWg?t_'ÛvÀÊ?ŠÍó4âØ?"²ïJx?ïl_tYÄ?•u¿j{®S?£\f›0?®ÏÑd	‹?ºÂ¬Ò`Ý?µ£Ù;)¨™?ëmԟ)%"?¿B"ØOÀe?ÄC¿Ðîx!?¨êdÑ$›!?»äXÞØ+ê?¥]¾»?çr"ïé\z?±cUԌ¤?‡0¾V?µ°R™…·?ª±mÐø'? «[ÈYžÍ?é³'—'Q?¸ÂOZ?{¤"l¡?ƒÖ1d òÜ?ˆX÷10Œ?"×N°èÒ?ïgSRâó?˜Å«–'fz?ºÎڇå+?Þ¯ã²íS?Àöb¬aa3?´Ï4°0ÀÚ?èhŒa'ô?ÈÎw"®?Ð/š¾Co?±áµÂ8,?º"Îö¤?£Œ]*"a?ä¨"ÿ½T?³EU÷¥µÔ?ÊØáÁw?º¸™,?Ï?µÿê`¥j?œÄAÊµ?æ©?Ê£ÛE?¼V:OTHER3FGL J2038.8-3613@"o›™NÀB5™€o&)À9§ßV<L·À;ªÍv?ø>¿¼'ZqKØØ@
@6Tû¯ä@•P?ÞgT¿ä'@Ö½o¿ã	F? ô¿éÛIq&ù¿ä×›¡KUNASNone?í‡)nR?´&…¶†æï?£_jž¯?©¤×Ã(?«êa+jÇ1?ª9ἕj?î,)FJg,?³2¢˜"ï?ýS·¾ñã? ¹|»vêì?¥>©ú4Æ?«þ]¥ó½?ë•1ë_‰þ?©• µž†3?§ÕÎėÌ?"j~ …K?·Ð¿Y2&?£ê±ÿWi?갍ãFj?­ƒ·'	$?¢²ÙS?œKöbBKq?À'0?ªMð†Œâ×?ï=Ö:ðÒø?nb…Ç"Ø?€¶"Àà²?ŽŸ1cCT?Óݐ¨ÿõ?"`OZ˜?ïoœo">¶?™-…ÃO«?v·>MÌQ?‡?ý¤ŽÆ?ˆ½Dïs?é?'7ßÛÁ^?î§Ç2•9Ê?Œž&¡Hr\?'Á珝w?€c€NI-?™WÊð"K?ƒ¶,{ám?XM‡?‹ëyèVµ?€çPU0ʪ?oÖC…»i?Ÿ"¬Ì†"É?‰yE™ÅÁôAGN3FGL J2039.7+1237@L¿/˜sÿ¬À12vd
k"À:`ýŸÓo~À;®QC¿rq¿õÃ{胷…@ò…¶Æ'@Ç«_ê¡I¿æ÷쌡¿í"ccÉöP?ÔÝ!yJf¿í˜[¿Õ~³UNASNone?îµÉ†Nì«?®íûm?`WE!¢[?cbæåâ?£óLf«ž?­Ë¨#c÷?ï4vqBÚ½?™$6pHu6?{»¿q5–?†P=ÅK?''BZ²¤?"b"äûO"?êd*ý.¿[?¨#¶(öH?µÍÉð $h? B¬6¥µ?·Þ%ûí@? °Dþ?îÊ|
þ¬?¤, ÀW?;©[ñ ƒ?U|œ‰?,?£ ìgOx?¤°'䱋?ï
H–Ô?©xoÇEöÆ?eæl€Äî?x2/ß·ý/?›'IgGÏÝ?©öHŸ•­?d—Íì?~ÎC-Êé?bõ>˜-"&?di*Gp'?wÃDÞ÷à?w·''y^?ìj£Àl ?¤|Ác»?±Ð'Îý³Ý?›eAüŽVQ?«'µœG?™ynq?ïÁ'w¥9F?xÈn¢Àü?,	c;›¯ò?5º ã˝??~^y
—ƒv?xOøj±6AGN3FGL J2042.3-5416@u{êüÎXÀBÞj㣨çÀ: jOÿò"À;¼àm"¿å±ÿ~GP@
¤ќj@lŠ I6¿â‰	Ú
¿ç"¡ì#¿éky˞¿ïû:%•»¿UNASNone?ïÙHꐾ:?s	ӓ
ÿ?W«Ú¥,¾³?Y2£Âò–Q?já(­æÒ?mà†(jÜ?ú±=?¤¾ôî̽?†€è•!²$?Œ> §3mè?¡dV/¦O¤? ìx¡—ãä?íÂ¥»·?•¨§²Á†?¢*Æb®?‰Æ…æF?¡µÅÜ.á?ŠUž2©¢0?ìVÌR֒?§gÚ¦F~©?–	Ö6¤?"M%B?·Ç:ÍÂ|M?¤]Ú@qÂâ?ïç#$>Æ?…
'[?SÂ?n?lÿOžÖFØ?]÷x"7"?~UEŒÍò?¾¾l7?†U¿ô#T?lïÚò×Z?lQ á:À?'_	å®Þa?'kZ)؎?îËSH…š?"Üô ôxU?—l
ÿ³5?|wJI-P/?ŽúUÌ.O?t]ªw"¾8?ï+œæÖ
h?†3¬µ[?lD_d™Nœ?f/~23þ?—×;jÙ ?…ÝÞ]'AGN3FGL J2043.6+0001@GNE^®âÀ8¸*º¾­OÀ:•sÔãòƒÀ;µ¤(hÔÖ?ëiG¡K·@
Ô爏Ü?ûÚ>ÐJ[?ÔSÙI:&?˜,Ɵ›˜ ?Èïx?Ï¿ãòJéÄe†UNASNone?ï*·<}ðØ?±Be2è=I?sZóŒAPß?A—Y`_	?•Ò[ÅEÊ?¬Äþ'[æ:?î}a?¬ã°]
I?"òª à²H?Ÿœ4ñ§·?¤Ù¡AdÁ?£Õ¢¯Z½?ít–Ÿ(? ø`̹û'?¡ÉÂ'sÝ?"gS f?¦ìÔ"=?•eƝ!¨5?í!Aý)?¯ÀüƒŽù?•}å$?œ‡ªÔ‹zK?±–®¢1¸?ªî&+c ?ïWȨœ?¸Ô'¼µçÿ?p'ž´qp`?"®"ñ$M›?ýº¸}S?´tª6þ¨?ïG´rôûP?–š%¾R!?€·'ì™ù=?ƒQ¬lCmé?[Q]¶V£?YvPÚ²?îâØ]µÎë?º˜¨éÿÊ?' ±
o"y?ƒ±Čÿ.?'"C8gd8?ƒqw‰÷ג?î¼4c´Û>?"•ïAìq?–É€¾¶œz?Š@±IYRf?'¯òÃÎÿ?†E·ýÚLAAGN3FGL J2043.8-4801@uúw1ÅÀC!²_c<æÀ9¢îRX'hÀ;³ Œgï?ññ[!ŽÆ@|¶M"m8@ó‰à%¢¿åŸGŒí ¿Êx=3<B{¿æVH«•p¿ïÿÜ^o³UNASNone?ÃÜ+žG?ÁråZ?C?æ?Á¯jïÁ?ʛ
€×^?Ã$á+(¢¶?ÃîõáÃÿÊ?«N֍!ˆ?¶Ï­Ó''²?ç%¡Ï•vl?ÊG‡~¨Á?̕Ã*ëð?Ä·NØ¢?ق¿e¹ Ô?µ&%]Ñz?Ú·0쏓d?µV<aU›?nj[m—'?¬çòm_¨?ÂËMÑoð?¯Sä»x^?ènL{Ê?·®½cÀr5?¶ùúè$R?¨Øºdìóò?Ém™Zqš?Å<Ìdž?ån[¼$š$?̨ÖÅÁb?ÀØ÷µP%Õ?ÁáE¦c'³?¼âDt‹?ÁúWgè>?æßE¿kª?Ê	ïܶ»?ÆäàP‹?¹lq;ñ6¨?äh¨^i¨÷?±ƒ'†<á?Ñ+ŽµK7?®Û>÷Ùã-?¸žÔß3å? Øz~A¦?ÙwÐ?³RuÈÍòc?á3*´•s?µ,NxÅ?°ˆ{Ûå¢?œOڈÍ¢MIXED3FGL J2044.0+1035@L)©~+VÀ32;yRÒ5À:r‰ŠWÝÀ;– f<tû?èݗÿÕQš@Fýo,Æ@S§`Ÿþ¿Æ
 œO#¿å¶ˆSåÊ¿ÙKY¥bЅ¿ïÿûC¾×ÓUNASNone?îó¬NõRõ?®œ·o7?šõ'À½‰‰?­
"Ì?zSÍ|àÿF?‹ÌyY?êúö…Ž?½&&°BþW?±Þ>ERH?¯ZŒ'l?·pÑìtÇ?´T9²ç?é\n?p$Î?¬ö¼'ˆè?»ßøù{?¤©G·%:?¹<•ݖ–?¦7O8ןÕ?êXUÃHc?±H5¥¯˜?¯pDk×Îå?¥¨?àÑͤ?½…/²Ó¯ô?©
šâãÈ8?ïˆáG]?¤ýývÊB?†æ!¾ˆê´?¡²»Àrè?k†d±ÿÓ?"|¯J}I?íjô<tÇÊ?°ÎöMÈ·t?£è>õk?£,Gép?¥h}A0ñ?¢Tø%§?±?ë%[•c:H?¨ŽŽ"&ð?µÈQØñ»r?¡÷ŽŽÅøj?±Ñ}¬@J?¡ú3›åƒ?í˜Ëý³¹D?–-(:p£?¦ð ¬&qÖ? ¯7É-?Ÿ>ï"%Í?Š3<Œ'AGN3FGL J2045.6-6838@t`⡵ÇÎÀA¶Ü­¡À:kYnLÀ;¸à°¯_Ô?Äõ¿&,K@‰³*º=Ô@$¿²‡ý¿âú©/tóÙ¿ã'ú±À	£¿âê
ªþÆÅ¿ïÿóºÄ®éUNASNone?ï&ï&$=2?¡×3´'?wÑ2f÷\K?‹©ÍT˜Cê?•-Ρ6'¥?žÍ¸D-?îa\;j9Z?¢Y@/?‹r×ZfË3?‰Tr—"ü?£
†qæЙ?Þ†'1ɯ?ì…räà?¤\q5›o?ªìDÑàÐ?š׎™×?¬Ãyè©k,?žóI$Ÿ?í4u*Nˆ#? A›ùí­?—˜õlĝ€?ŒËLݶò?°vS¤r?šÅ0¡mÞ?ï€å÷áÆ?¡C
h?ÑÊ?f¤ti'0?€6~sxÊ£?ŠeEmü?ŸyÓ*´ßp?ïn
uD·?ˆ$Ü¥ª@}?w´ðÁb§?qÆg}q«£?ˆ¡Ä‹_Å
?ƒÌÓáö¡?íÁ—I)·?¡S¼á('?¡[éìµxÝ?"WàkÙû†?¢Š¡ƒBÌ ?š3;o+Å?ï=6ÌgC¨?€£X¢=?Ó" Â™t?oBô¡8?Žß*8ƒ?{™(㪆AGN3FGL J2046.7-4259@vaŸ!-w2ÀCV4XÍÀ:mGÞ»ãÀ;Íw=N?(?Ö>éÜ°£@
ã͍@T kDò¿ç›s³¿×|žjÓwP¿×ƒ¤a–v¿è_¤]ö]óUNASNone?ïàŽæbJ"?ië]C@‰??Pyç©pFý?S¯¸jAH¿?g4%÷¸j4?e6VOwù?î­Ç¤wv¸?ž®5Ðûi?"êè,(ñÊ?…/£uLÖ?ŸÑ—UÕF.?™jÏÏ(œ?º¾,v?Ž†¾ÆZßù?:7Ú,?éb'h?,¾ž¥?†)2–d·¹?íˆ/íêç?ŸS´Ñç…?a*œž¢;?‡§ÉbS!?¯LkϘp?šáAô£Ô?ïó,ö‹Àœ?Qí«Á›µ?8ǧ3Œ ?68C¢"$À?StN"¾i?NzÆåÊÙç?Ô[ü?ƒ 'OÓ¸?o¥P÷\J?h`+ ­?'足3?~ÿÇ5](Ö?ï\L¼FB?~u!ˆÇ}?€ìÊÆx?rÙíyš«?‡ô*xj?u¡
b[mN?ï2é_»¸?€Á'?…ÍãóæßK?o™:ú«ðó?wÄ'yÑ?wwØpsÍAGN3FGL J2047.9-3119@)©IÆónøÀB°>ž¡À9Äz•ÈSÁÀ;«zl­¨D?ê…ªÉÜq@RÊ/cšÚ@*zàEûb¿êþLÂY	¿á[_Ñïó¿ã"Åãà Ð¿Ü˛Lª±"UNASNone?廊Je?…	ÆJä?r¢…ÍöÆ?tƒ%5"÷??{	mzIw¹?~"¸	fô?î¦äµ°'?©Øÿ¨Î2?…¦ó‡?"y78 cë? (¬ã+?£4˜f}]Z?í´óM{D?¡TþÀ'†?¥¨Æ‰·?–ÐâÉðÐ?¨«ê=ÆÁ?'K¸þXª?ëòä>Œ
m?¬Au遲t?¡0¨¢øH? öÁÍFC?·Ð‰¼Im?¦ñ,{Ô¥?ïЀi$_?säþª:?aãL弪ç?ctÚp.?mœIÓWÞ=?j~gòd™?ïŠv¨ν?"»¥¿	A?q}IÒêòŸ?€O´Ì6?"£±#ÅA?%2LU˜?îÿӗÂ)?‹ÜÑó?aÇ?@…~b9?"Ðà1øXh?‹è–R?xÌ0C¹n?îÂögÙ`¸?ktZTf2?"2ŸwoœG?")Ë+ŽV?"n""C"¿?…8xõ譇AGN3FGL J2053.1+6027@XV'Ìö¾8@$"òsPÀ9KŽÀøƒ4À;S"9-H8¿"ø¨ÀŒ°@&§}‡ë@W§Å¬¿ä¦!'ÕbÑ¿çÃOÍ¥¿¿è_¯ðjƒ#¿ä͚ŽGgUNASNone	?ï%`J–?¬Ä%ÀK7 ?~ `Ac¢?€·K:£Û`?"«åžYw?¬i±Z¼ @?íä¬-[?¿‹¸|ÖÝ?˜=qX:‡?£¥àµóþ{?±J‹CFz?¹"WÿP?ìV¤ø{?¤âÞ²Øxà?žœ+Ïy•ç?‹Á°Î?µ£ÍJH-?¢±)S›?é¹£¦I¦?¬X–w|î? R'@?"w~¨Ù}?Äõ\ãÛ²?ªÌ$è4	Ü?셴¿%D?Ò<ú•:—ß?[mý4¤Ç}?de~=¬a?»d£‹¾mA?ÒE"p´ëQ?ï &AóF?¥=P¿÷V'?L‡—_iß?"J|pB¬?"Tô!VR?Û›
­i?î«[QE©?'2¬½5Ú?Íòÿ??ýì™Ò?œ¯OÑ^?ŽÄ‰F
1y?î?^®GaÐ?Ž.ÞWHx?ƒdË@6¥#?n"ù»¤Þ?§0âM¡û;?‹þîï¿AGN3FGL J2053.4-4052?íUÅߝ´ÜÀCä¦">jÀ:Yt^v­ÜÀ;Òù=¼¿Ä©ñÍڋI@4؃9Zë@TF__áè¿ä—I$_þ¿ß/.©9¸¿â†g1ßÃl¿ïÿÀtFEVUNASNone?îm¢<ÖJ$?¥°Ð»ö?‹4Š©Å>l?Š¾lŒÆ!?¢X¹…–Y(?£-f·rä?í‹2	?ª']FIhé?˜ã%tpÐ?—c
Ï{?«?œ‰IP'?£òû#|?éÒõö?­Z.¶Öÿ?¼îµë3ë?¤ñêË\ה?´ú¼.?¡"FMÑ ð?ìK'ёi?¤‡±Ç…1¥?¢,Böl$ä?˜}W!Wœ'?´']Hc#Ä?ŸÀèÙkî?ï+Yü"a?¡(ó¨Ô?~ò¿·"ß?™òû«> ?'ØìWµ&?"ÂAavƒ?ïE¾´"?2\ì_Ò?€3ˆD‹a?{—ZÙó'?Ž\öc¼2?‡ŠÎ§»]?ìÑv¤Ö? ß¼¶Y$?±×ËÎsa?›–Ér´¯?¢såØËÙ?êýWp?ïTՑ¹É?"îzn8Ë?…D¯m§‰ƒ?u⩐¯%¢?""
'͘0?t󳝧AGN3FGL J2053.9+2922@RWâCV—À#»
QøXÀ9ÖV>Ðö'À;V±AV¥?óÙ£A«q@ŸÝq§?ø²€@LÜ¿á훨´â?ïþpßÍ@Ì?ÊGɉ1¨«¿Ùµíkí}¶UNASNone?ãÑù,&Nž?ÍVáRÇ¥?¢"\;W?¢ÁW¬Å?Öl–ðá™?ÍR@mót?è«nf)?Ëíß8ž?«ôZ‡ðU¼?­a/Ä›?ÆVƒ¢êÙ±?Ç
ÿ¥š·Y?æ×½N³?·_âê㑟?¹
×Ù;™?£h¥<î{?ÈØ:ò£?µò.TRòÔ?ì&P¬?ä?¶ú5&š¡ì?ª—ÖáM¸E?¯±ÉÁH˜?±ƒÚ?V½?°ûò}"9?éåä('¢?Åöåvøì?œ²–!§?œée
¦	?Æbœ§ô"?'n䁳?ìíyû#†?¼íqŒN[?››ðb³fe?ž,LÜt&?±­4¬H¹?·&®7ì6?ëXíò·B!?ª†`a&§?®j#''ûµ?šmËûæ?¶~Ÿú# ?¦l¼¢ÐR?í~Mø¨À ?£ª-&Þùç?¬Çó×Ð!p?ž†ßqƒê ?–¦Y;G¹.?'¢Ûò
3AGN3FGL J2054.3+6907@Zð¿\£@.Ÿ¾˜V£{À9ìÆ%鞕À;¤¡pþoÝ?Þ>ü³"	s@¶Š{C˜0@ªx z´Q¿ì8¦O¾ò¿—rÍËüøw¿í£­n¸š¿æ@²ôDÇUNASNone?í?ó^m.é?¹•Î|¨?´F{,6¸Ð?¹N¯ÁàEâ?{žžš¦ƒ?ƒbÖO´ž…?éaQ´BN?ÊÝÓkˆ ^?¿µ¬¨GºÝ?ÁnD$Т?µ?ʊ2¶?½:Yz5?ì$¹y]å?¤'
ß;–,?¨þ–c"Fù?–Vg2½,?²_Çì_?ŸQŠ‡?ÞD%Q{Ñ:?ÚWã{t?Ûm9a~?ÆnåÕ¡ ?¹;{s¡?®Á¿¨w?
>?•þ
ƒîƒù?‰2@!¶¼ž?"Ke~ëà'?j˜õ›'W@?v—™` ¥?îí"\]?¸š¢MÔ?Ÿ®Ð&bY*?¨bzH›zD?',9…7?­¹ÿÀý?îzîèDfP?"­ EV?–
¥Þ<?†¨s0Œ*i?š—}Wùð?‹´Ùãw
r?ë*þB)Š?§ñÞ°ù'a?¼4÷«?¥QŠÜôT?¥+ÿrsœ?"v"ìË1AGN3FGL J2054.8-4908@uâ'RT`ªÀD‹«`kÀ:?ø³o.À;¹wD;Ï¿ùAž‹EîÍ@P!ˆ¬6@ސ>&¿ê%£"˜ÅM¿çLèdi_¿ÎB×Ë®iµ¿ê"gƒqäõUNASNone?ïõ·Áf«õ?P5$qÊ?@;{Ð #Ý?9®0¤="–?HåSg2'?HÛØé'K?ï'éÖë+)?‰-Æ´EF¥?hx˜Éä/Ø?tD
ÜÕëô?‰'d
%#Ï?ƒ^FÕÛ?î64d-'?• ¥'õ`j?•‡\Œ:9?Å*T±ð?¢vŸ×Ä?Pr*·0%?ïTPa
ÙT?‹9»Áep?+2‡"ò?7:W€Ê{?•?ŽÓpiš?‹>"?ïú@rƒLž?=©_nJ¬?4!Ñc;?*ƒiº|?9ÛTPÄ{‹?5ˆš"¸|?ï×õ1<Zq?m;Ÿ¢Îõ½?S•°~J?QÃù‰Ú7?n?öŽñ?gk0hE?ïIA\Á¡ö?ÉE?…w™û¥c?r@´Ë~
?ˆ8Æ3®î?uu'0 ?ïÛøsïò?båpD§?l!t5<b?áÐæŽ@(?q¾žP¤:?b¾%çއžAGN3FGL J2055.6+1609@OlUÚ'(cÀ2KÈâ\
À:+òËdÀ;¢Y£àDy¿ó7‡mò÷¯@
‹fNJBº@ö_ÊëÌ¿ç
y]0¿éØyti¿â=Œ˜TJ/¿à\¢ÿã"SUNASNone?ï¯Mò•øê?ˆž¹Q
'½?8֣¿¼?;4¨õs\^?ƒeÎDª×•?ˆK
yÝdë?ïUޙÜh)?"÷˜H"èê?ss7ÔO?|.=Rr?g_©OH?'±DO/?í5"siÑw?ž.¯Â…3!?˜éäy€ŽJ?ƒïO2?°sEã]4?™‰9Ls‹?îóñÏïº?Ž"ó‹W«p?=(d½{-ß?=·­o—‡s? †'6ëýÔ?é¥§m7~?ᅬG¹°™?±L²¦<š?&É¢Üh¸R?$åf'&iÑ?'øS}?±M@å‹P$?ïÊê×FDÕ?vFhýjŽ?Zͳ͙$?ZñGˆYE6?s×'«'þý?rŽ»±|Ó?îù#ԊJ5?Šî`ÿøˆ?‡é‡ˆÊ?|o)[«Õ?•U©{¦ú?…õN"dº?ïÊu¥Q;e?f
\Ÿ×Ó?"57
Þ?.cLshŒ?z3ƒ˜Võ™?eÚu~°ÛAGN3FGL J2056.3-5925@u6;%oüÀCm'Èâ]À:*¤L{ÖÀ;áà'ód?ò'ål€Ü´@óùˆl '@ir"¢?¶rj5òµ¿ãDè›pšƒ¿æ¦üP¿ïÿÒ`_'5UNASNone?×Â#¨žÄ?ÉåçÝÁ´?Õàžã|Þð?ÊÿfYœ?Ò]=såL?Ëüøá?ÄlY
·?¿	:?°³Ö?áÞ[¯B6?ɦ»|SžÊ?Ò3'tóX8?®:%âe?ݽ'A8?¶ªrây?׳‡»d‰[?¶•*ê§?ŵŠ2jÙ?¬ñDj,Š?ÎÀ·º/Õõ?±ù‰!r¶?ãúÑÔv?¸qú¸%G?ÁUþø3?«Ç¿Åð¹?àûTÐøç™?ÌM2\bpQ?ÏWu²µ?ÇJly•?Ìû™d¦®ç?Ç°V	ˆ%?Ö.‰‰ðÈï?Å:.ÜÙ¬§?ÝÓ
wь"?Ç–'kˆ?ÇüÑü{Tú?´8¶¾ ?C?åäa"\ú
?°±×ÝÇÒÚ?ͅYh˜?¬Ô~l$Œ?µÒA"Í•?Ÿ',ô»åZ?á<¦à4?°¨CÀ?ٟ¥äÍìÕ?®î…_Ix?°çƒ7{™?›HžžHý`MIXED3FGL J2058.0+4347@U@dÜY2¿ó¬§
£3À8$óĈ[À:È	€²B?Ú¶óƒè#ã@݊µ%;@\¥ÀC|'¿ç;	XØݿ뎵jZ'Ç¿ïþh#¼?ï½IÓnãŸUNASNone?ä³¥ñ©L?Ñ{Ø0¶´»?«°ûP1?²?Ø "ªY?Ó"²U
?ÐE–çQw0?ϸW0'?ÔXHm¤j¥?±•°Ý¬8Æ?·Ð1Ü?åß4 #b?ÓDzüÂø?ß{AÖ F?¹Z™ ‡eä?Æ)&ÈtV?«ói	Ýõ?ÕR*Å%?¶wèïÃô?éÄÃï·+?ÅØ"Ð^Ó?Ñ'*¶Õ? n*:r3ý?ÇÏ×/ô†Ç?şE¤LG?é't¥'?Êۋ'L0k?~A¢­VŸ?•¨wA¥ÈÄ?ÈIPDÕ·?ÉòÌΘ?ÔVx¼C+"?×yi¾4®ˆ?²wS£ˆ?³ƒkTUÐi?ã…á·¦±?ՙ÷ƒÀÐ{?ç¦å`R·C?°©UóSS¢?·säzfÄ?¡å«Ìê,n?ŪxA¸º¥?«ha¨?î©Èí³ç?¦¾ïæÊ^?LÓ$
9?hޛ}3?¤ûá=Ô?¦¨Õ,ùfMIXED3FGL J2058.3+3729@T
™E¶ÃÀ†wc
ìRÀ90/JpfšÀ;;Ð<ÃÕ­?åðÑgñq@
ÝâÃJb@šåÀŽ¥ö¿íÀ°º¦L¿æz[>¦?+¿ÞèúÇÔ6ñ¿â]Àc÷	UNASNone	?îμë?)?žÃ,%}?ƒ«6©•?…µ§¼þì?œ™(%P+?™®Q'@Æö?à:uJ?Ó»ñ¢?¹›Ï¶®t¿?µÑ¸cÇL?ÙxϞ}û?дè-ë›?ëÒ3q¥?¦½ƒ5''w?©..Ã`22?"<£²<̼?ºòWæ×\?¡ûV8v&?樅~ÉM€?¹,Ȳ	G¿?¯–E2VlÞ?§ýÁ`g?ÍxX¹!Ç?·"¥ÛíG?ïrãö›8'?þ!ꜧ§?td9—O?qÿû8*£?‰;u­ôGû?ˆg8}¿H?èo{$'kn?Î_®•˜òÄ?«g¤=?­OnBÌÚï?Çzy‹å¯z?É^b¿pvh?îN'ÿÃçm?"¶äæ,Œ?–3gðÛóý?‡ØêOZ)n?Ÿú8ºS?‰÷éW³Jd?ì51À¨?£@»d£ ?§h¸°'E?'Æ	 Mùï?²¢ÒhÈ4o? 
DnhAGN3FGL J2059.9+2029@PÇQ'©"À0}°5½Q/À9öÚ˓À;…OºRvÅ¿ú&"î9.@hÛkv¹@œàŸ©¿ã²ÍN@ą¿ìr‹FÖº¿ßëtbS¿áÈAŽDUNASNone?ïqJ³,'°?'¹®€_ƒ?E§b$fÅØ?Eú¾ÃÕ0?')nŒ›F|?'ubä˜ôÃ?ï1ĖŒ~?Ÿ•â¶á+"?yÈ.E£N?†.'·zØ?";/Õ%y?˜áðJ€VÒ?ì|1B÷ˆ?¥_Œý ®?šäž¥?†þ&š¬;?µeO\îõ??¢lš?î)Œ7Ó£?ÌµO؅h?>p¨¦lŸ*?@-mçè?®@…îK_•?±sST}ë?ïÍ矿?~s¸×Êô/?3)óPØð–?7g"qLà?wِÖڞC?}"M>tn?ïÄ؝C$ö?|Ê:ŽUʋ?^"ç{%ò?bî|‡þ?uò¯•psg?vSgH &?îðæNìï?…¡†tn?"j½Õ5l?p${^uJ?—ÝÔü^?'FD¯Â?ï'ó%Î?v¼w¿Ú—?ë¹2o˜Ô?¡ %piå?‹_UÜó?v¢>*AGN3FGL J2100.6-7844@s£Á½¥À@W±B,Ë:À:vë»ÛÀ;¨¥º9LR¿Õè6W!qa@éÙM
Ð@Ú]ÿ—¸¿ëF|ˆ‰m¿èⰠě¦¿ãš&É\C½¿Ý"¤[OÃUNASNone?ïúûä'fJ?C¢ÛYÐÔ?#ô¨ËW¿²?)×µ´Ô•?>&ˆÅˆªý?@jiRñhß?ï|žVö9‹?‹ï÷ŽU™?jF""ùò?tÁ©¤oÞ¥?ŠFé-œ?†œý|BØ?î¦D4¸C~?Œ‡¡Sà?Š¸†ùì±?uŠ¡›Ð?Û5êIi¾?‡&á
ã?ï!¯Ä˜Ä?‹öãšÆI¹?Jû©'ÁuŸ?L…T2ECI?šò*µÒ°?‹{<î:3A?ïüÙ¦¾´ö?<ÉÌì-%?á"\¶Õ?&w'¢.J?2zdÓDÝ>?5À†ý‡»P?ïÔxìê"K?o^cÓYé?Týr s4û?Qañn»=?p",É,q]?iÙÕzl–û?ïw‡Óô^a?wfÉÕÏê^?y…4ÜýXÈ?gô©Œ=
?…[pœ¨ËC?r_5¥•Y¦?ïÖ=
;\?e-ÛtIA×?6ÈÞ´?)À–<…‡À?stì曞?d—ö¶"AGN3FGL J2102.8+4704@V:§›ºÜ?Òë|eVFÀ9]»JÄIqÀ:üÅCk›?é/ÇÛ÷7/@ŠaÎQ1@'ÿ\—¿åև¶¼©¿ÈšUÅô¿ãQ˜ahÙ;¿â«RyÓYUNASNone?é=TYüÿ"?ÃB$[:?‹-`:œ@å?‡ù¨?R:?ÉWؕ>&h?Ãf-0À?µ€V3#ª?Àá.}è?¹Ã{Œµ§å?°aò¥é"?ꍢæŽ?Ä;lãG?é-ÚQMX+?²K)Nåt?®æ7IEØÍ?œkϝ;ك?Ïç/N¢?®ØÀˆNm?å𘝴ö?¶½ôQR?¶^ÿ+ÿD?§NxɤÖ?Ð4_VÝÃ?´Mµ«]?í"gj6C?µTZ"œs?r^ìÇÑ?p…~y–™?¶Mvû,é?µ5Éud?ÇO•Èr?Ð[à°Xo?ºŸ¢æ'}?¨9'_nº?æØ&19€L?Ïòx–G]??íÅrÃõk? b1aA¦x?šŒ¾®•Ãæ?Œb<YNZ>?ªIåcS?šgÄzçÔo?ê&dz Q'?¤/'®‡¬ ?±Öwè¼8ø?•Ž‡iØk?¼ödBA:?ŸnvS[MIXED3FGL J2104.7+2113@Q <K	êÀ0çr>á½À:\%ĵ§À;¤¬°Í"À¾|¥-Ì@Hÿœ'Ø@iÀÎO?ã߻зNG¿Õïãð!]¿èñ¾
‰"4¿­t4Cú6ÛUNASNone?ïÏtE?r¾¿úɍ½?\V¬pŸ
?]»)i+ ?q`¬²…¹?op-C>?ïuÃ-36[?"Ñ¨‰˜?obA`	D?z¼¤!¼!?Š¶¤Mn÷?ÞWL›y?íÆÿ4lÝé?–Ý–c­—?œž‹Œç?‹ Q3mMˆ?¥@Ç,1?ŽÊï	à?ï|³Â²?ŽÆrwND?
¹01ðÇ?)Oeh ?U|÷1Q?ŽºUè"t?ïë9ÙYfè?`ðAá?ER	j™N?Gu_¡Ü¬?^ãISZ.?[¦$÷A#¼?ïÔSÞñ´Û?s… X'C?V†[YY?U°Êm¸ô?pRï
lD?pQD©ßò?ï‹K0w?"{šÁg?³ÿ¬>?|óë0Mm?Ÿ¹6ð?xþŽ>³K?ïè¡2F?b<qšÖìE>άSîž>Ö"?"¾aC?gWn^©ïØ?b:T˜;SFAGN3FGL J2107.1+2248@Q…£Â‡èÀ0V2.oÀ9ýE= óÀ;‡ÙRMI¿æå®Zk@
"÷P®ï@Ïã ¡5D¿æ–
ìZdX¿ç ^F~¶â¿è™•Rë'é¿×}‡TUNASNone?ïvÛîË¿?'øœ
±&P?`we2ýâÓ?aÛäuÀ‹s?Ž++xWu?Ãð<ñ?ï²ó?¡-ÊóÁž¿?zšÖýʓ?†ƒ~ÉÒ?•cànë?›ÿÓìC
0?ìû
'ç¿?¡'¼1Ž?TÕ(í³B?†þ:E/»Ù?°Òv¡³H¶?œC,×LÎ'?î"û"÷?™6¼eݐ¦?]·uH"®ÿ?_é…EŠ?¬â"SAm?˜ë
™_{Õ?ïßë-?r2Û¬Þú³?EWóyŠC?GׁÉ?$?j¿H©4?pk´|É}+?ï½8åϨ?•ôõB?a1"Ìsܪ?fÊÈ.»%ò?xÊʛô'"?{u)
D«?ïmB'e?¹–mvòA?ˆ7M˜:ÿ?r'qˆÓ(ª?'V°Þ&2ç?x†‹=–ÿ'?¯üåø?sD$.òÏ?>V½¤"ìÅ?2Q"ŸÀ?ˆ&^Õie?rüôX¿ GAGN3FGL J2108.1+5202@WTów[@ÒÜʵ›À8n†º™ÄbÀ:³×û뿼« ÜrËé@/îWŒ@v7]d¿ßëŸTR¿êöò·åV~¿ä¦ª™q*»¿îݓ»Ö}UNASNone?âJÜ]A,N?ÉMƒ>kÿ
?Áƒ•r9ü?½[ã¢ôƒ—?Ò¨Âû×k%?É	yñˆ˜ë?âèýàɌ"?Ñ:ÊÙW ?µ¢ÚÚr ?²Ñ=Ȗþ?ÔÅ}ǚ͐?Ìî@ÿ"bb?Ù½¢¦S?·ˆ#HC5–?Í
PÍÙ?²Ó­­?×»Ž±‰$?·¡ZƜ_?Ý+K§¢?¹˜0`*f?«23¾OYÐ? ùG\¾z'?ß{Ž<sd?º§n2Qz¶?çqÓµ…o?Çn±t½Ó?¿©ŠŽŸü›?¾¨vc+ù?Âg'iÙëø?ŽÐ˜?ê‰Þªg??Ç
Q:Î?§õã1Fª?­a8¨Û.?¿¼'oýá9?ÀӅä"ª?ä'Ã?³t×®­F?ÅÄt÷×E)?¬›@E'ðÞ?Éقûûìþ?­ê‹d!½•?å¥Gp¾^?²!ùÀnò0?›K,¬¹år?‹ñŽÓ6??Ó¾TA©K?±Í¼%.ŽMIXED3FGL J2109.4+1437@OØ$>úèÀ5áŸâÚUÀ9NØ9¦ëÀ;"wÏDvÀ`Z"°ÔI@|p¿…¼m@ÜŸ‰Ê¿å>KïA¿ì²HČXá¿â"ÿ½ÿ™B¿æUÂ`ˆ7UNASNone?ïü¥8øÞ½?9DËgÁp>øè$eÓ?>ôEãÅ$ç?9G·Ï^n?8ÚóäÌØþ?ï'§æ
'?‹™ä–bł?j͘p?uÏyb]~?…2ÏBðUî?…-~GÁ?îÊÔ¹ø(?o¹#â?~LdQµ2?f]ÆiM?ŸO¼?†µ?ŽbÚ!/?ïÚúŠS?rÆùˆžrè>áÂPý&®S>÷Âêo1?rñ!£èIÏ?r–x2ä?ïþÌÅs›?,$+U¡>øêv)î>ò[bŒ¼
ç?,%ó2Ê?+V•6"?ïÚHe@îÕ?pQ–~?Sè‹‡A¯?R˜ÁÐj÷%?kï¦z­b%?j9ó–c!ï?ïs=FSî·?'»'d´q?oϤV*ÀÞ?\
MþÉ?‹<ÅX9R?'f]/ò"0?ïùgzì

?Há¬;]}>¬íöÓìv>Öhp&–¸É?JZ×êzv?H® 
rAGN3FGL J2110.0+0442@Kx"ÄGÃ
À;Ö2.oÀ:;÷ƒY¼4À;³{ë2éa¿á&æxFä@³ªÎJP[@cŸâˆ÷¿à¸94
§¿åEø(<¬¿Ù
´ë?寿ګ贒vîUNASNone?ïúG|Éݸ?9U…EpÔc?7ǃËÆ?
$5j¾?D[!NÇÕ?7´I"Ic^?ï'@«°Œ>?Œ3?êÉŒ?kø‰O»§?tâ0¶Õe?ˆqÏv…?‡­¬õ?ï-…BZԞ?'¦jj;?'0£Õø?ueeÚÚ<†?'7/!´8?yö‡>vÕï?ïUÉæ×Õ?ÔöñrK]?3ÇQ-°P?5ê—éä`?"÷Á4k¬?§cú*ôå?ïýNÙyP?'™-¼š8!?
$•×K†Š?Y&5"?3ÈôØÍW?%|FEë¸?ïÖé¾l"?n;îlŠå?UuNsóó"?R+ߨ®Ì½?o0oxº6?hyc·&'?í?«^?qþŃ"?u
w¥Š>?n¡ÚtAþ£?|È#J«?aN{vã?ïÞ5\ƒ9?Y»ù4f?%¼4"¼á"?7Á+t'n?pIƒ¶<?\?Y%óaƒAGN3FGL J2110.4+5946@X-Œ*EN@Þ͍¼ì…À9W/ ×{|À;5(ö™Nñ?ÏM٘žX+@'Ë+·é¼@EKYl-¿çõ[s"x¿ïē_e7µ?ëçÖ4÷Ñ¿ìÊÒ @3ÄUNASNone?íÐÉËTk?°ÞO³ÊÜØ?IÍZd›"?''
fÝÅô?ªÎ|œ«a?®º¼i°?èÉ¿ÇU¿z?ÏÞ\tӚ$?´xŸÿÞHÕ?Án†zMh?œ°áp.?ÅßiÝiR)?è¿üŽ%?¯
l+ׇ+?¹p\Hö$?¢7<óŸv2?ÀGß½•LX?¦»EÍo?êNÛý¨?ÆQ–!âJZ?†¸Š‹äÄ?¤ŸM­?Ä?7šÃ]?Śé-‰-Ä?1X?§àލОÐ?ŠÒ²6jí?‹ƒe"3?žÿƒ<ç»0?¥S£b'"¸?é¶îßFL?Ñl<»êsÉ?»Ñ lج?Ènh'9D‰?¶vè›´H?ÀXð5vs>?ëß¿LuhQ?¤¯½ÈM?°e¼nòW?š"å¼ä Ÿ?°œI,†Ö$?š¼£&¯C?î,ðý"Ñð?°(Š:eˆn?‰ÛQlP®?›´¦‰n?¦Ì¹PŸþÙ?©–½i
ýAGN3FGL J2115.2+1215@OM'#[NÛÀ8scä«æ£À:¯çÜôÀ;§Þ7X[â?×:m-n¼æ@6W'¸ÿ»@JN LO¿ã°Ì)Au¿é"Æ gƒ¿Ù¼%UÿÝJ{ñŠiUNASNone?ï»Qtøâ?'c´Ô·=¡?:®šãmå?GÊ	Þi>?€j6à}âç?Á¾Õ'	:?ï,ÐTãÿf?šB*˜­T?xNÆF~Ê?|"SÀòD?"RCÎôµÃ?—1'ˆÙ ü?îm—À{†?'1À<Q²?‹}4Æà?up"Îl÷²?¢N¿8Œ#ê?Ž¿à–ˆa?íØ[ ²	?œ½ÒG°Ï³?rõ$0>?v.ÓáÊý?°"ªÅ~?›I‹ƒ9,ˆ?ï×I-y™?œ©;€ï?=ÍWðR?mA¶™W?r~—·û… ?™Í©VÃ?﹂±[éF?€åՔÁøn?b‡rxŒ‡?bh©zÍҌ?yúíôÉâ?|‹é?º¤?ïlB'®?x¶R.}?z,v•…{;?eU™·dh?‡Ù mjÏ?s×uC?ïz0¸A?y–=¹Ä?lš'žïP?_ºîUQM?ŠMXg9?vkÙ¥ŸÍ•AGN3FGL J2116.2+4422@Uél <K
À
=›l±À9ŠáçDòÀ;J¼¼´Q?ê¶çnþTH@
œÚ–Ž¢@ô÷í¿î°±A𪿿ӺãÒ^¿ç(þ'jöï¿Ñrž<W8UNASNone?èÛ`ßqr½?Ï
›ìQš?ÄkôÝY"M?Àž*|D8?°MK;ÿ?®/gŸ»±?Ý>°§´Ã?Õeµ;‹œ?¶{6DZ<Ë?¸,‡QÖR?Ý"¦?Ó+'l8˜?çÊ6§ÜÓU?±Š!¾ïþü?¾9ȑ?§H.ã…Zy?Áº—|D/k?¦SÂy?çÌýj,?¿<™ZÑÕ?´–ö[ç\p?µ%ZK?Ƅc)‰Ö?¹±?p¶Ôñ?ë";b<ò5?¿ø]V>È_?»|Ñs
õ¹?»æTž=?¦â¦ð H?¤œ<ç0-?æ¿Ü#?Ó.n?©pó°Ç?°ê&{1')?ΤR£Cš?ÐÄ°"ˆ?ì×Ä{Dš?¡œÍ…N$?©ätKeàÙ?—ƒCkå?¨«ol	îŠ?"n.zÊs?ìÁcâþgz?¥¨Ýà>›Q?¤øŠ$b‰-?šý|ý]Œ™?®ñ7©ÿ1=? ¶p,¢©AGN3FGL J2116.9+1343@P	:¼"peÀ7Ü¢G'ÝÀ:/–WZZÀ;£æÎ-¿ü½¡'	Ó@ä–'IE@ØÍ¿àVôï^OÊ¿ã²íáx-¿á}-eeé¿ê™Š]ÅUNASNone?ïDkÎ@{?'…ë/ò°?»¡xx¶?¨Aœ2?)kZØBì?Šz¶N×?ï8–"¬té?›q•á¬—s?wmý¸•ÆÆ?'˜ìI?"­ýSÓ<?–|ôås "?쪟ÙØ,?¢À>ýth?­¡)ÀI¯í?˜Ã§gÁ
?± žs-?–ÙU=÷5?îTá.%$?›àŠÞ?W.ïӋN?\ÕCy¦?©þq­d?›‹^Uf]?ï̓™¥X?vk_ùՎ{?ckàL&6Z?c¢CÕvx?pBóS?o¯x1¦'?ïÆ-úö<?ylª¬n?]…üÁ¢›M?ZÂ(~ƒNŽ?u‡ƒoF@ú?u¦ˌ?þLݺ?Ž.Ö`/§?–ƒ¡y{°¿?†P	–Á?•K^¼è—ó?~€CW{»…?ï™+ÇGìm?y8íNMô?,€d(MJÄ?1¦í)Óð:?‰C"8
ñ?y
²-HAGN3FGL J2118.3+5751@XcR?gôÜ@¥XÂ8õÀ9pËæÀ;d ;ë¿Ô³"î'̉@ÙM(§¾ö@Ýé_—e¿æf"suÿ¿èƒ¤ª™Ç¿ÞXœóg¿é)÷ŒáFÏUNASNone?ïVâã­˜?"¹×׶Ãs?€\s=xR?~N[¸¢?Š2ê¾aÈ?R…=Tï?í©/Ü!?º'þ0-UŠ?‹"-¾Ø'?'*´°¨ª?´0ÉD®»?¸E†C#áÊ?ìc­KI¡×?¤:ƒÃPÌ?£Ež
ÕR?'M­¥»®?³\òÕb,!?Ÿž'Ðó:.?êÐq]¡'?«§õ|ï>è?}W%ì¦Äi?r|el›}­?ÃӁZ;=v?«(eD•k?ïÚ¼6|"Ï?nuv³h]D?aË7å_@Þ?^ô+¡Z˜?cx'¿	/Ÿ?cé–HŒ¤Ô?ï1sÔÒÄw? ¿{¥n¸:?sV?؀/Ë?u8"6ÿS±?"ûõtÚÊ?óõoS+?îဍ{v?i¦Ž~ñ=?H4³L.h?ƒ¡0Ñ»h?•á›C›hÚ?…*G¶©É?î8ˆ¸˜/?Z$"[Ô?p¸†®ú?\:T0wÖ?ªhÕà¼?Ž»P¦öaAGN3FGL J2120.4-1256@Cxéö©?ÀCmS?B5/À9Ô¢ç 5*À;µšTbX?äìwþÐfF@È'qßÁ@" ©ƒG¿âD4ҏµ¿ê*¯8¿æ"J®êu¿ïöEI5SUNASNone?ïå*e'ð?eM¦`Ý?Pfr|։Ÿ?U{%Pù˜	?b¢az'"4?_%"´B?íXUŽtCì?«ÜdhŒÖ?š!L؀6?˜f£
Ö4?­j©çþ(?¥…|÷ºp±?î°&lŒi?Œ™~³Ó?"ë7¯ç?AÙ?•15Ñ?"Ã-´³õ?êÅý`q?ªH8)Ça™?¯h®…³
?™âf­'0|?º`£êç{?¥Å{õ™Ê—?ïï»)6Z/?dD:{«¹Ù?JFÄeG¬?aú.	ÀL?SfJÛp&¢?Lq>»X§ ?îöÅ÷›'}?"yìÉûß?‰#P:u´Ç?'ެáæ©?"•˜òÄqù?Œ'z¹Ç›ç?ïLˆYÞÌ1?{?¯Vfy?Šm¨
Ë{±?s"ÙûR?'pAp2¤	?p-=Ǹ?î]DÞE4?p÷jî?œ18jÏ?€EôÌ0H?˜%Óÿ:!?‡ë­§\i§AGN3FGL J2121.5-8253@sXm›äÍuÀ?M>EþÀ9ð¹£$\×À;q©Ä[åÀåèô>×@
T"ÆK(r@¤S_ùdÛ¿æ!Á½"ã'¿è…sä˓‰¿àpÓþ"ù¿éÏÐøFUNASNone?îåaþð?£|âT'?lýÙvá®:?'Î]9¤¹?Ÿ½Ø'qÄù?¡jQjX}?ï~ô…ߎ­?1'BÞN?jÀ…"Eœ?vLþ ,÷T?‰'½"oÝ?‡>ñ¢_?ìoHP?£ÈÍHaM?¡½øºåS?‹zÐ;îÎ?³¦Á"q/r?Ÿ—Çä±(?î¦ØÞö<? ìIâô—Ç?'Äçy4?7sµžÂ?¥z­(ïAÕ? æFT#øë?ﰛÆÅvÂ? ¥¥"†4.?cÀPãèb?Ÿ·¥—U{ð?}Ñôö²?"
4>©µ?ï×eñeL?oÞ)*Ak?TUÌ}Ví?U°›õ± á?n»³¸'LÛ?hÃLTD5q?îâÜW%<?†Û0'
+?ŒˆGNc[?x=¬Í?ƺ?•`Y@"îÛ?~ù•Brò`?ï©a?W{3?~_÷ VÀ`>ôdÜpô*e?
tÛÝL~Ã?…}²eöÝ?~ZÛ)ŽAGN3FGL J2127.1-5615@u9EÁ?ÐÐÀEÎtŸM¡À:QéõÒ"À;ÇæÿëÀH•7µ#
@
ô6¯"'®@""¿æzšûÄ\¿é¥Ù	·¿Ò³:«ˆÀ•¿ïÿÁ£›G'UNASNone?ïa¦ù~†™?˜1¦×tåh?J@üµ¼4?P©?!Ӎ?'ùïµæô?—õfŠã?ï‡RLSÐ?Š—Ã~åü-?h"6~ö¹Þ?y¯&·bvÿ?ˆ"ßQTs"?ƒ$àž®ú?ëéš{õá?¤ѳÈÏ?ª`­¼&¼?"mÖžÿÄ?³'ëPr=? k‹rÈ#?ïuʞž†?'H±¡Wü? ûz[Ò?7ä˃X[?'& F¿©?'5à‰-•Ù?ï¬;
Xi_?‡}",&·j?H±ðÂ
™?I""£ù-?ƒf¶­ƒ?†÷ÞåXÁ?ïÙâ_ú3?lÖl,QÙC?RŒßh÷	?QÕ¢,'ã«?l×u3©"?ft­®#ìP?íî°¿Gu'?"É:ažØ'? '¬ñRL°?…ëŽW;é? ƒG¢¦6?Ž/–IÅ?ïä0¡¦?kȺªD'q>é9¸òš'?F·?k¶²d,ي?kÁRùR¸ôAGN3FGL J2127.5-6001@tê"ã¼Ó[ÀE:â–êÀ:Ç©Á/	ÙÀ<
œKû¿çš¼s°ž:@2"YŽ'©?ÿ5ºŸM¸›¿ç<íyÉ"¿Ï+@Ç+´J¿æú~˜®¯x¿Ìÿ)UNASNone?ï߅f†Ç°?jfœ'Ê?BÈJ¿C7š?@<çõ«M"?kȆ"ðÉ¿?iwµûd°?ï_žæàtI?–]t:¿'?py_®6—À?'Þÿqë ?Û–u?º?YɚÊ8v?îU¡¤¢X§?'/Uhú?'` ö"ÿ?cT–Û;?¡uÕ88þ?ˆ~´G1{?ïÕI0~?"Ôô51ë?^fÀðè¸?cuw—Ž?š!!Cä´µ?ÍA?ïñ_çyÔá?TÀ[}¾Â?3kN÷öâ?0‹×¨N2?XepŠë°?S.k&FŽ?ïÑ°hjM?vÂihA¼r?V¶§'¿Þ?`ùˆéZc"?qzTE®¶8?p6"¼=9?ï=Ñýì²ú?|(>q[?"ÁÕ°ne?pÃÞ`×?‹É«kdc=?rG¬a$a¤?ïÙrvƒÙ®?e'4¨˜?5¼©¡ºkå?0\`d1Ë?qêú:"V¹?dVÌúù•AGN3FGL J2130.4-4237@vgxÔýó¶ÀGWzÃë|»À9ŒíÀb[?À;©Äe©?ìGœÌ vå@•¼ÚçB@}´"9¼¿ãçÀ¡lh¿è"ïjÓÕÍ¿èý("Oý¼¿ïÿ¨óz÷UNASNone?ïøá2À?Bøs6^?2"çùe!?0 EBZ'?Cç¸5èüx?<Ž†
…(?ïn¼=Þ\í?B§åúª²?mD?º'?v#Ø4§'?Œÿàœù¥'?†è˜¢|*ï?î…ðb†»y?'Ðô·'÷ì?›$ŸI?‡Ñ]ý¢‡É?".Ï"ñ"?"ÝÅ6Ž.?ïjø¿Íh‡?Œø€z{֗?kRj'\t?l¯9¨"´?Ž~;jmB?Š¼…*AŠ?ï÷țå¤4?…™ß	œ?E
*¸™Ô?…+ªðÝb?7¦Ê¬è?C§º—á ©?ïÌ.W^ê$?scµç—ü#?[)ió+?X½Â8Õs?s#ÉÛñð?må—"Ý+?ï¦$'¸½?'s¹	ESê?'Yªˆ'¯˜?x¼$y€ V?…c!ï[E‹?tã"ܜKA?ïÞ¿\»†˜?jŽyMÄè?W¡Ž+6šˆ?Q42pÅW?eoÜYyB]?g)MšªH8AGN3FGL J2131.1-6625@tjD›¥ãTÀD#")³úÀ9¦*Í3$À;Õ8¶*?òŽ1^FÝ4@©X†~߯@""_öŠ¶¿Ùî)òJhb¿ä¸pL¡ÌÌ¿éÔÑß8貿ïÿä•|¯UNASNone?å#ê)÷A¸?Ëg˜€|?Ò:Ûàïw?Ê·œP¥Q?«í^|\þÑ?®\ÑÌñ?ÔÖο|hm?Å2s3˜"?ÙÃg
US?ÇÞ·T"U~?ÑeÊ3.D{?¾>.R½?âЏvÍ^:?¶1.¶3ɪ?ÒõþNÏñÅ?´9¥Ô~?½£‹UG?¢ðH25ì¨?Ù{R=±Þ¬?µ†h¨·¤?Þõ(¹»*Á?¶E–8ñK"?¾>"KÚI?­†Ç‹ÃÌ?黩ë1¢ö?Ä7h•f¡?ÄEʺxâ?ÂêGéÅù@?¤<Jԃ?£ïZTj(?à8uvh€â?ƚ®µ"'î?ÕT"÷¦À?ÄѯjfPA?Äuä7|>?±êe
²Ñ?éš"m}?«u8"Ë,?Â+§Åù–Q?¦â_m.?­±_Øß}õ?—Êu> ?çºH?¬'KY¦¬«?Î4G}'?§ƒˆþ®j?¦N!&ì?šLG¬<MIXED3FGL J2131.5+2605@S"wškP±À2F£"¯WÀ:)ë°½¢À;ƒŽÝ}ôø¿Û™Œ;Ê@óÝq	Øq@(¹_\±Ý?ï×*æ!va¿çÎk·mv¿åé{ÜÅ=a¿¶¿µÑ_búUNASNone?ï{C<b(a?"Ÿµ»®ÚX?`;¦˜\b?c‡ôGš? GA^ÏV?"
žÈ.aÐ?ï7}ŠÜé?¡QûÖ?uÉóÞÇf«?	paÔë±?"ÑÈÆ>$?žQK¬c¼6?í|´í™1? ï‹ë;? žcl†Çø?ECÀ™ï?®éÑDŸ¤ó?˜Ù»®Óy?íDÅJˆ ‰?©Ì­ª3?`L¥¡Äô?hè–7R'J?µTëFûá?©¤Në2?ïà^ `Œw?t?ðk'!?C³¶ï( ?GÒ`ù´F?j´ñûa¶?s"Ò±û?ïÂ5ã¢ãV?7_Ž˜ (?^_2q¦?]«–'šI1?wMA‹js¾?{%§·òÿ?îæ2хæ?ˆÀÓ$¶¶?Ž"¤ŽÊp˜?|ÇS_òœ?"ïӎ½/'?€ûî=¬Ô?ïu®«?ƒoTÓJ~?Aºg¥ï?=ì×þvYé?Á¿ÓjÙ?ƒ?ÿÑ/RÁAGN3FGL J2133.6+2821@S£ëJwÀ1Q\éåâÀ:*`	UXÀ;›•]ʶr¿ñsp/g÷‹@¤ž™ˆ§¯@üɀ'±¿ã>úµ?	¿éòµht2¿ç–]Ê¿Ðô˜PæšUNASNone?ïÜ~a–H?uÄoš½g?SÇ=³–"G?`+ ­0+?iÿi¶Í?r«'Ç«`þ?ïZs¿{'?—H@jç$?s¯rËÛÕc?€G§¨]Ô2? é«;â?'—†Áf~?íTƒw:Ái?š'xÚv?—*kWt­'?†ˆ7V	u??¯"'Þݤ?–¶»È«p€?ïM"!Ns? ‰R²¡?6_—Õ>l?<7]ò°?\φ²À?Ž‹ÚË?ïîúmI?cûÓG%³?>j€°ë©?Hä=b¡x?ZÝ긺V?a`B_žê?ïÍ·ä{õ?ui¹PV?Yï–8V¬·?[4:»%V?r¨((š?pèZ'Vñª?î»ã±üÎ?'
Ÿ©¶²?Žø²©ÅÒ?†¶¶¢ùE¥?™0ƨb¹?Š²ÚÒ+Øâ?ïÕS:~oá?dÊø€ìŽÞ?R´Aù»?ÿÑ*x¾Ú?u	 öY?d§âõ'š AGN3FGL J2134.5-2131@<ëÊû;u!ÀFŠœË}AtÀ9H£ÝÀ:À;¨jJ÷u¿ùñª—˜¸s@¥P+¼q`@`M¿Ø"9Ùô¿æaaÍX¿àâÍú–«ö¿Òéå,XèUNASNone?ï¡Ý~†ÿÊ?'ì^Šh?P'0¾«?K²Líó§?…ƒºQx'C?ûÎÖÞç¶?ïˆ|½Z?‹[¥×»I_?f†ëÂ]i‡?u)á¦$ζ?ˆX¥ùóMI?"¹,%‹Ô?îPζÔ4m?'L=Šù8?"8¯<ü².?'etô6È? Ö¼ø‰ã?‰…¹V½ã?ïÛÜ4HÝ?'7ôWP*?"!äJÿ—ú?)¦ój*ÄZ?œÀ@µBe­?',ýÄNi"?ïãcJ¹Gñ?g`æ¶_"|??²å´gÆ?A>wn%i?h¦XÄe=Ó?dèÊ$k
5?ïÙ$ßæã'?pk—2ÎÓ?Rr`y£>8?TÎO¾#©?m¡ï³%?iˆt{MŽ^?ïe·'(7?zó$¬U?^¯§éº?r9ƘÏö?…Œ¼ÏDD?m,MÒ Ñ?ïÔeaÐ÷Ì?g9|øH˜>ú+ýêöNA>øbeYf?u³#œþš?g.~ìbÊìAGN3FGL J2135.6+5742@XÆÂÎFI@ҒwcåÀ9Zžˆã—À;ëóف¿®×¶Ý7®6@)nu©z@ÀôÌùî¿ça
ߤb¿îM:piI›¿Á.Õu½ÇK¿ÒA»X¨…UNASNone?ïƒêxâÈj?˜SK"øG±?F<Α~lÒ?Eµa‰ãú¾?¡"êÒ)*?˜'4é°w?ꞅ #²ž?Ν ÂmM`?ŽþÒû²_Û?—æû"cäQ?ÕüO¶‹?̲M‰d‡?ë1jԒÇv?¬yc«67? O«iô½?"•«,Ñà¬?¾LÓ¥%‹L?¨ÍiZۚz?íaÐ&ô`?¨£Gx|¢ð?HÑè	?UË×Ãl?´Áy$·¢ø?¨—´™ÓÚ?ïÖoñ³Ç?†˜j»!ä?<f¾Û‡w›?@Gd¹ýXN?s›Nc/?†3Û1'?î'ã ßð&?»@̖ú‹€?xë-ºÀ1;?ŽuIÙÿ‡?£Ä`8A=w?·øgU/Ï?íÅçÇ5Dl? '/'ýà?‹ú"sS£…?'§ÃU~±?¬¢Þ­Ch?žbÙPš ?ïP1õV¿æ?‡}¤ì? *?I3æþ]?AâòJp?•0(éb—•?‡?<ÏëÅsAGN3FGL J2138.2-4939@uÀE¡ÊÀƒÀGyÔbÃC·À:,õXQÀ;^ç$?âíÊ$"w@q†žj9@W*?nªÙ¿â¼V¹ä×t¿èª9G@Ô¿æ¼þ'"¿ïùÚmZ‡œUNASNone?ï§^Eہq?ƒ÷锄`?u¦Š'uFÆ?|è6rcÎ?vªR«FàÒ?s¦K-¾ì?íü1ƒ—?¯…ìê?œbÕ?ë…þ?™Ø"(¥º?°jTèÈ?§•"4Áý?ìÐ ,"ü7?¡=0F ¡–?¬xƒHš.²?—ö9±S–?¦…yñÆqã?'^bµ!¢w?ælµ,òý8?²lê9õ84?·Sj"Ð5?£ñ nY€Î?ÊÍ–ê#?¯o‹²'?ïÝXoF£—?kÒ=µ"M;?b¤E'î?cú––"?`›ì®EŠ?Z;kÅÓ	?ï·SÇZü?"'QG~?"	t	Ê~ž?€:$¨p©?'d[€K˜C?ŒÌŽ»
@?¡»š?Œ©ÊÐY…i?œ¢ú$û‹G?†‹‡RÝ,?Ç¡èót?v휬=S?ì-–±æJ*?š
c΃®?ª¦D1d$b?‹»æ¬ ?±@(X÷ƒ~?"p*!¡dAGN3FGL J2139.5+3919@UÐ?'æFñÀ#бx³pÀ9›ó÷´$À;}ý¬h©?ð¥\ürÖ@+ƶ³/î@ƒ¦¹Ù«¿ëÑâÔ1V¿å'Á³`Œ¿àª­<±¹¿ã>›¥ÂUNASNone	?ìc|7ø®—?¹‡?9Úô?wBV¼¥7?ŸD©ØJC?µ†M©¯zý?´æ"ð£§Ì?æ^LÆ©?ÐVÛlUqT?³GÑ;¹—û?´ŸZâoõ?ÌâäJ[²?ʊr0eÑ?éæðaHç?­^¯¤"'«?´¿îµ-^?œàåÆ^lÊ?¼Á½
s1·?¥šøÆU?è6I@÷Ó?¶¼rɍ!?¶ÐÉigŽ	?±Ë5ÿÞu€?þvGÚà?¯hØ|E…L?î*y÷Eyå?©™ä˜öz~?"ÒzO–/?•,·)]­–?¢ï#gLæ?¢&Xzݚ9?ì&ÙÒ³…m?ÂÀó·áó?¡²$fýë?§¥)˜öI?µð8œ­	?¼×fP8t?í¢â7d'ž?œÂ¦µ—ï?¢]Š|Ý>?']ü˜>6?£tR~¦Cä?''Æ,#éL?ì€ÌvÄ5,?¢Q7`V'c?±¼h*g°ß?IgZµ¶¹?¤zh@¥|?'³<u)·YAGN3FGL J2142.6-2029@?$i@5z5ÀGG@Ý?á—À:å¡Ý4ùÝÀ;Ά"W£?ä¤õ߯lY@
Ö3=o!K?ø[6CÌÞ¿ÜàÃ2f§¿à"ð&½ü¿ïÿƒb½?ïÿH
úƒXUNASNone?ïvÚtL¥?›"mÂ3?oÔV•v;÷?wŽáÓÆÆ`?‡­3»ƒª?™yËHhb?ïyûàqÖm?›Q¨¿&q?l?Ña8?ˆœØýØi€?Šq€ŸÔo?'QY)‹}?ì/××uzß?¤·<ö¶~?«ê±±ŠÉj?ÛAöÃ?°‹èiÖöV?8&}'R?î¡<lþ ?­cïòs'?i¿é)ÆÃ3?‰§Ôâô@)?¤P@ZCK?¬Ž"¬£º?ïʾOäøE?æÇYLJÒ?Rñ,9Z?`¯™'%?uä3fe?Œ²u*þ?ïО®ßÚy?‡?:k<?[inCU›b?v¦^žzå³?pÖLðŸ?yNö
ÈUÑ?íĂ
(Dd?žQä½Ý°?¢€=•÷?—o
"à0?¡7À^
Å?'àÇEQv?ïÖÀüŽh?~CžÔêû?B¢s¾þû?bîÇY	¢?r\ͦ0"¿?{"Ž}Ý:AGN3FGL J2142.7+1957@Rnì€Ç:½À8dv}4ßÀ:±<¼M#À;ÝGP ©Ä¿âjaj©9@
Ü7ùÁx@ÆÿXeG¿î(ÂX¿Þÿhd‡,ô?Æ;4}¸	¿çxšö]UNASNone?ïésÒñ»*?j½®vsml?.µ"¯¬Ûó?4¾+,Ÿ´?d ÔÉ2õß?hØ/#ª@?ïO'Ib?'´áaTß?u¨%ýÛ?z7±ÎíÚ?­ë¨]–Y?ŽäÇvhëf?î±@Q©ÀÙ?‰YáIÕ–?‰h$¿mŒÍ?tå-¡
î?#ãp8ˆn?"IM^(›?ï>Eq½÷6?"Û‰Ö6a?I¹T™Ì·;?Xmcd
7?—i‡qôà?"ƒ¢Ö<Û?ïôyvZòŒ?`'…"Üö? I[°L~?=ÈÑéÉo?Uç‹þ{?`k™ÄsJB?ïǟ.—?uèèu@' ?^íI¢ëçÂ?Z¯ÎšóX?tuvÒÜ?q–ÊAå (?ïiTŸêk™?sÞ%áW?{v´/[?aý¢³ÃÄ??‡ïvùd8?oKá?IÉ?ïÖ蚑Cè?h+L)dU}?B¡ïÞ%Ü?AûdL»?r7tƆx´?eÿ"¼˜Ï&AGN3FGL J2144.6-5640@u8}¿HÀFßÓÃa@À:œF&Tþ_À;¹ÌÏQ‹?êÔ¥ý¼?@až½c£@¨j¥§š¿ë'FcM¿ìdG"EL?¸YØxýlÓ¿Æ\Z®î"UNASNone?ïÞÀØLÝ©?ræ};Ä?D-˜D±Éè?FÈ«Ò&E¦?l3ÁÕ£74?pÏËûy?ïoʹTÓu?•"Z5B¼o?m°FhËï£?€'{lÌn?Œ¡@!é	?/ژ-?ì¸Îg£õŠ? »é2…¤Ÿ?£"ɵ—?"5³æ?°oªýða?–îìŒè?î,åU§Þ?ª Öç?jò(ÿü?‰aFYA»?«…oƒ*^?©{â÷ÌùÅ?ïàÉǒXæ?jhóìÛ6?CêŽ üì?BÔ×MyJ?j;"¶ôÞæ?gðžÈ1yv?ïÑrŒB ¿?v°óùo—?WŽdVˤ"?`ÌVÓöá?qc åi'ü?p1xõ"?î²#kžè?†8ў;ì?'bƒ[î?…&fœKœ?˜Y‰
	¬?ƒyځ×3@?ï–÷uæ?ˆ!©TÔ?kæã×.ëE?tHšÎ8?ƒH".ʂ?"j‹»äãAGN3FGL J2144.6+6606@Za¼@ŽÉ@#ˆdüÀ9Óz¬nˆtÀ;ŠÎû{6ÀQ*3d>@7å´™@¤ÿŸÝÖ_¿èz^ò\¿æ¥6û꜖¿ê‰Q"Eä*¿³Ô~.õ…UNASNone?îÈ	ˆ{?«Äg'sUC?{p¯ôY˜ ?}"OÍ~½? ©iô?ªÕåhä?î‡é""Þ/?µÊJP+?tÞћ¹e"?(µf߁?¤åŒ…`±Ù?´sbŒâÝø?ëí4XC°P?¦ºÉÀò˜?£A=lZÞ?'‡‹ön?¶õ¾ˆÿR?¢bÌp49?ï,œ®L9?•«Á'Ã?"gÿm?¹Ìâ"#?šb|RùÝ?•¨"Y$
Å?ïI"ü{ç?¹U%RHB?aÞ#J%Î?cåÃôKæ?"'œJ$?¹p` Ô?ï¨ó¡b?',`^¤ ?`ó®¢8#[?w'HߛE;?†,Ú_¬?ŒÿU÷]Ž?î¢2­¯Ù«?'6›&õRÌ?9æmÂ,3?¸Âþq!?›Ãájt?‹!Nn?ïШÜ؈˜?lÜÙ(Æ>ÓÐéýI¦>Ô¡ÿÎÍÊá?w¦o.d?lÚљy†ÿAGN3FGL J2145.5+1007@Pƒ:'£À?‰Å«âqÀ:žÉã%ÕÀ;ºF"
q?ØøšJŸ@
%Â4‰´?ø××?A‰b¿ïĸ#G'Ë?èF"y&²q?´pUñÍ¿ºî‰FKz
UNASNone?ïîö'J??b/
±–.æ?)Ù¡Nîjš?'·ëÏt¨?^×ÆùÃÚ?a˜»x;¥ó?ïw<Ù¾çv?Ë<G
?mL•PÿâÒ?vPý/(+?ŠÝ¤.Ÿ¯ñ?ˆ$ݛVQ?îO"6Ÿ¾?"rÃ2F?‰ z˂‡Ë?víÁß-*?¤Ç	µb,?"nŽO¤Þ?ïeó‹—<6?'fçcœ?^Ǔ&¶Á©?h{µ èŵ?'UV	",?'—‡ÔFÕ?ïðl¿pî«?"õ>íí°?"b²%2üS?B¼aÑÉ?\Ú*e|¯?"°Ù7z{Ø?ïÓà‡Ã?pô¢ÚƒW?UüU³"a?R<"OQt?pªÜ†Ùñ?kýÁiõŝ?ï5ø6 è?…D?++UX?~Ë3©R"¿?pˆ$™ÂÕ?'Ž,Qb`W?ƒ_­imã?ïÕ.+ü!?l7ño)¿¨?X–n…Œ?SVäk¹‡W?n'³ß<O?h!¤»,AGN3FGL J2147.2+4730c@Wnõs}¦Àk¢æIvÀ9"La…VÀ;6É5h—™?ãÓä(^@
Vu´¶@w‹¿ç60¿â(ÙcÅ2‹¿åûhk¤=â¿è¢'ð'ßn¿ïþŠ¿·¡UNASNone8?â"7³z?Ĭ›O¸`??Ãۘ¢MÈ5?»£¿oÏò?Ðéù@Ñ´ò?Á °wŠ-É?ÀîŸMŸ?Ây%)t|?Õý.æº?ÀßÆüÃ?àÅáÌ
_9?Æ©‰=xRï?æ8»¬Øªj?°åmŸÄ½?ÁýŸ]Rìa?¦»Ü¼?ÅqïJiõ?§¨kZÌ<J?Ö1§ÂÒ"!?°³P²œ‹A?Öb|ùó?µêT©òύ?ÓkÛC:Å×?².üõb÷?é~א9€?¾BûäM®?·À(´(ÿ?²'egNH?¼IÈz¥?³@NTÅÖÄ?Öz
³\Z?ÏsŽ•ã	X?Ñ	@0þ>?¼z½F® u?Ø|µ8Â¥h?ÈyÓËď?ë‹CF•r?¤<;Z@‹?³¦W¬GØ?šª™»
T-?¯ÿ>Ù*?–^ü'jÞâ?ãÌØ›£?©±'0_0w?ËQÿ©:mÜ?¨,ŽZI˜=?ÅzŸèWº?¡º•þ""MIXED3FGL J2150.5-1754@AѺ^5?}ÀGºCªy»®À9¯[¿PãÀ;¸@p"Í¿¿J‡C3d@\>ø8`o@Evå¿èFì‡'Q¿ìÜìÌéË¿ÜMÓ4<j¿é	¿ônž¼UNASNone?ïçäp,Ó?j9DÁd\¡?Eº%1Šy?G̤«N"?b­G'œÂ?fÒØiâìz?ï7[æ¨›?"q‹h?t"†
Ï?yü§×Z${?"^JƒÉÞ?ÈÄ5–¾2?îƒñ"D"®?'k j¡½?ˆÏ—àË¡?wÿ%Åìô?¡!"Oæ;?ÒˆF·©¸?î"ðæž?›x¤ß
?oÐô«ŒUü?g{Î3?­º¡².ö??šç<9Â?ïô‡¸NC?a7&Š®?6:Õ@ë?<@©yœµ>?R2;£y¶?\Ùûv'à@?ïÃ&B+k
?uÈöä—
?^‰'VTƒ?YB–3ýÃC?vÊzLvJ?qئÌg_%?ïqŽ_}?{ó]ÂFð?wA­ªö?e@£Yé°?ˆ
÷F?xtø<I¬Ñ?‡œ
Š?vÈé!Dñ?]ÁzÜu¸?I·Îàª?‡Ÿn·òì?uoéG°ÜjAGN3FGL J2151.6+4154@V­ó¶E¡ËÀ"åÈ23XóÀ9°ÏS(œÀ;jV9Èxª?ç;™|Ïo¦@(ZÅ4¨?ý"ˆ`Xy?ïÅÛýþYH?Á7†""0ý¿áö7™¿Ñ—ÔtAUNASNone?î' &•YÞ?±ñóš¦eÙ?:¢"õ-?×»(º¨@?¥h¬KSä¤?°Q\
ý:ý?é"Cÿ_O?Ï¡M¼-y?¬Ÿ\!û
¹?µþÅl /?ÂÇ´– ?Ç X$¯6å?ìéwÍìÝc? _òç3? –]š§ðü?ŒÕ*L+h?°iÁZé?™+´cÊTÍ?äkþ[:8`?¿¡iK¸?Ã^^ã˜Ê?½
}‡jB?Ë:¨43…¶?¹þ%×F?ï¾²ð?ºÛÞ¸‡›j?è™¶¼Áo? bý(ϼ?•'ÛN5f@?´2X%ºÈ?í¤%}Ð?ÐÆJ$?XÙ}7ÍÇ?¬SÇ1À2?°t¨u¡å?ºdÆ9pö?îô8°ý×?†ªAlìÃ?‹#ËÊñ?xHY'¿Í?"øX뤩?€©Ïã%Ö^?ë¬+ xI?¦'3
Ó?­@ZM©V%?œ™9P?³þuÖå¸(?¡Ƹ"9;AGN3FGL J2153.9+6626@Zž†ƒ<`@"ÚÚUK‹ðÀ9²Š½]ÄÀ;%ôß:›¿Ù]W…3A\@–"t¼@5_®ç4?źÚ
fпàWågÎE¿îÀ°^×ý?¯#³=£‡UNASNone?êf0š–]"?Á±'P",?¼Ó ˆ^f?»Þ͈.Á?¯öµYŒºî?´£^'Ì>ß?íû[#£Yr?¶üîÀ4Œ?†îwú?"¿ÒâgH!?ª¦Òôœ]?³õ³'<xÄ?èÊç_J=f?¯—¥rØÊ?´Gv"é[p? 'Äéœ?°§ru=o?«2摁ã"?ëÙ¯ës4?³ OÛÔ_?~5pÝà0Ý?‹Ú)_R~†?¿T‹ri•?³4·«/r?îŽÐÛOF?ªŸÖ5üó?—ÑLq^%?Ÿœ/9î')?–T˜+Ýë?¡v¹$6?ï…£o?•€½·Å¤?lš;¹Â>‹?s(a4+¸a?‰OŸ.ìÃ?'ÔIütñt?ퟣ@XØ?žãS	b?¤ŒR4/{{?'à¤ñ"?©Ù³"[[	?—u"OÚh)?ïå‰Bo¢?'Ð炓jA?QYdœ©?Pô8|k[ÿ?ž¸"û]?'¢K'ý'›AGN3FGL J2200.0-6930@tö"Fs'ÀD{ꁺÀ9°Úx†ú[À;À‡»JÄI¿Ýjá€Õ@
µ"}¥ó@Î
Ÿ–2Ý¿éŽýCô¿à7ðeiwy¿éÛ(I+¿ì9Š¹	ªUNASNone?è7O%ñÅï?ÃÍ6u?ÈÝóc˜~?ÁÊcÏ:îÇ?©@;M?©äèg;?í&ôrÐyw?µÖúeEÛÖ?œVͤR?¤"ç}.'P?¯e«Ô¥Kc?®kS¼?é÷^
Í8'?©ð$Ã=]Ø?ºrLc/û?¡Qœ]å?µÒÃEøMR?ŸÞ²ÖÁ;?ê~cw(D?±¹»‹Òsº?­²ŽÅ?¨ê
ŽcW?½3ßDbtX?©¡ø@v›E?ëâ
×Òí×?¼pp\aD?ºÎ+Ã8Šœ?¸s|‰?˜…õøÀ¸?Jº‰4?ï=~Éx?›EÊOôþÓ?€4£ýsÿC?ˆÌÚ.wF9?5Úaȸd?"feaDÑ?í+ÿx+ò?ž$#xìU?­oa^?˜NuZðÈ? Déâà?‰»xâKˆ?îËŸ?R!"æ?yM­â˜½?zéhû]·?àXuõ?Œù»B`Í AGN3FGL J2205.9-4704@uàÛv³¼ÀJ•=êFZÀ:RhDŒ÷ËÀ;ç&p­F?㋖͝"_@
¡rŒÖ@OÀ A¿ì@%"0›v¿çÿ–VKÄ­¿Ô›ã<óå¿ê??\¦
	UNASNone?ïÜË6cƒ!?o¦J=¤ý?X_	Áó?Z#Š›:]¾?g3B/f?gG±
[D?í»0؉(?±»–eÿÜ?–bÄÕ¹Y?œäÑ%wô?©?Á œ,Ç?§šÖÙ¶­?ìõúŠÌ?ž,¸D¬e?¡™64~ê?ŒP¡ù§…Ç?¯¢+:¢[?—
\ç8h?ëµ!4ƒ?±±z2
?£,xÑDx!?¡î¢gKþ+?¸TŒoÐÎ?«,vé[òÇ?ï¹Û™vçœ?®ámÿó?f
9N€@­?•B|EX¡B?x–­EÍ?¤Ó«LB½?ï;âC×p??—Uq¶ ™ñ?û˜o©«?…ùÜÕwy?Öú'zŠ?Œ"ý??îÐ3¸Oxt?‹"£¾Â6?Ï Å:Ñ?€â‹Çê$ú?•)è7µ™—?')½Î`*w?îšÕ¢"C?"6Lç;k?™in×Å?ˆáEb‡J?"¢éçtIÒ?ˆÖøIÓ2ÂAGN3FGL J2209.0+3652@V5*"8	À.ûBªŸ{[À9Ýã‹U38À;ª€÷â$M?Ä*½ðs@
¦zÐ֜¯@±Ø@žUÁ¿éùö˛@Û¿íÈnµ%¢¿É$ŒÅSd_¿ß&Yÿ»UNASNone?ï§È¿TœÃ?Š©õۄ¨?Gïû¥=?Hƒôr1@_?""ÏâM?ŠñÇÐ2?/
s?­í("Oý¼?…ග#?–ÒӋ¨¡<?úbø
?¦8l¡O?쩪Íåy?£¯Äwjz?˜e­Í»Ü¦?"'Ñ\ý§£?´™>%»·?¡;°oÉçj?í©£'Z¥?¦A'±É?q [uJ?y&ô¢'?±â¤õ?¥ÚNðº?ïÉþs?ÞÚ
Kœ??µíbn?AY}
p2T?y"ïAk ?}ÛÛ]‰H?ï•ÝónTÐ?˜/ՇeÍU?p"¡ý‰4Ê?‡ѳXµã?'>23¼—Œ?Œ3g½8?î¹3W<Ê-?'‡Tø_5?':מåAc?nÙ8r¢ö?Ÿ¼)Blײ?'ÛhLî»Í?ï~"²åù?'¡CSá,l?hGÅêg3?^¿(—t`…?ŠMô-"Æ?í‡å·‰AGN3FGL J2209.8-0450@K׺Âß
AÀFÇvõ׈À:--U£ "À;eÁsÓ6s?çÒR:èç¾@]ûÞ³)?ôA»¿3\#¿"¨ÚúîæV¿ã¾6ÿæX(këÔ?¶÷›CÈÆUNASNone?î\$»÷š?²AWlC7G?=öû'ÚÄ?C0#î],?ªƼ'öÂ?²AÚpó^ç?ï~[«þœ?Ž2	›òN?gäئ,¡Š?vHO‰†û'?ŠoÞýTh³?‡ØUÅn ?íH‰"7?ŸªÉwÏê?¥¾QŽ+ì?—
\í"W:?¥¹AӐ?"´—Ä#Ó;?ì|NÃî"?¶ŒÙI\A?lE¨KÓ.?{Q7¨ªWÿ?»;\ž!ÏÅ?¶c~˜uýê?ïêh'å?´·uœ–!‹?0Ј5­8?8G1ü¬þ?œ?pКC?´·âíNL?ïփZp—u?p¥?–4%?S…JàT?Q›AO+½m?oöb蘈_?kŒãþ?ª?ígìRE"?£Žbê?§éÌK˜eÚ?ês¥ûŒ?¡—n‹ÂÏ?˜*ÎåÊ­_?ï"øq°
c?":"'i?bÙꌏ;»?iÊ[kQ*í?™E´q	£/?'"t&ÿ"kAGN3FGL J2210.1+5925@YëäO QD@Àc'†WÀ8œzšÐÑ>À:æRxrØe?ìÌ;5œUG@0–Jښ@üVàŒr?¿á¸VCT¿éF'ì‹¿í¤ˆ3{闿îIšt¤±jUNASNone?Ú8ڜÄx?ËO¢2M?Û*q "Â?Îua
"Q?Å9g†2DÝ?ÄXÉV?Ëø)`»E€?É¢8•ƒñx?Ô@Ÿ•¾2?Äxì‰ðH?ÝÃL?Ÿ?Èÿ{?Äð?Ú'ÏÆ°?¸#$|1
?ÑXøÔŒ‡?²•¬}ùŠX?Ԉv)/¬É?´ÉL"×c?ƞ¨C¢äh?®Ý
(?<À?Ý9®éî?À©êiüÚ?×výA"£Þ?»°Žèí?â®'E%_?Ë+xUôu«?ÓnŒ¡IÍe?ÉôUaâ@?Àä,²2<?ÀÄ6ï3Æ?àòsU?ÑWA{±g?Ëø<¥€`@?Â&;und?Ñýý~<é7?ŎÀFExt?ä²ØL‡Ã?³ÆôU-Ø?Åù˜+t;Ö?©§–¿Ak?Ç;¢l¸ ?¬__wd˜?ÚX"¸´}?°<E"æ"â?ÒmP•Ä¢Ý?°Í#öqN?Ó:Œ²š5e?®	wD|~"MIXED3FGL J2210.1+6043@Z=îx@@AéÿãzŽÀ9Ë…ãpÀ:Ö8Ûé B?ÕÛNt®@gAžÛÍÇ@´ò€e–¿çý%ôËj¿ïÿíb»ÙW?ïüÎδü¿Ñ$|bßUNASNone?âQioA?Ñ\¥% ù?g=
l~z"?lª`GZµî?Û.³½îHÚ?Ñ_ó4"?ê+¯R,aw?ђ{Iļ?'"âX$YQ?¡³;f"{Ñ?Å,ælIîû?ÐxYMN<y?äîçeµ?ºÐãªe€?¯tö^%?žâhÝÔ?Óן2N '?º_㦔:?ê¼ñ'uö?Çÿ.k?N¤ÛlÑÓ0?rÜä}[¶
?Ä햆i¼?ÇøÜ[qQ?å]
¶º?϶­y}øÝ?`8Œk
H"?dÃã¥o{d?Õ%sykÉ?϶Ls²:‹?îaÒ<?Äþ6,Èò?}¾©Ü«?"ÜCڗ³?ªòR*|þ?Âæ"m¤?êx9cÆE?­ßÌ.Ç\®?Ÿ/uÇ)
@?'$Ü-ï¦?Â9¤b0²á?¬&û^(?î+qòƒ?²˄²³š?a
—¬±-È?tûé¦§?¬7_h q]?±²Œ‹'e‹AGN3FGL J2210.2+6509@ZÁøL­W¼@–*"Š>À9ƒžòžîmÀ:̍Wk÷ ?Ú¿Ýs–®5@áQ•sð@ϧŬ¿è'+f¾®…¿ëŽ´Ô©˜¿ç""
Ó2¿ÂÆ!{¿'ÑUNASNone?ä¥
êéX?Í©Ÿæ©‡?'7)WªEj?"81TÔö?Ւq"aº?͚T®ÇÂç?ì]çj›Ý?ÃYb˜Œºt?ÿèw¬?œùkåvÝ?¸Ðʓµì?Áñq¶•m?äÙÓ+È?·È-]$V?· í×ё?¤Í¢Åô2Æ?Ò¢×A+*?µÁŒ%2—?æ	¬¯©"?ÁžåˆÛ[[?‡¬'Ç·gŸ?'Y þ^\…?Ó‹h~n›?Á‰íaZ-?豩 \ë?Ë6¾¶'+?€ÚÝ:gÛ?†ž](+?Ì+«¬Ž
g?ÊÐDЉŠ?ï*\§ö©•?¨¦gÞ5ªÝ?ví%¼`ñ˜?ˆ/BªøÑ2?"ù!"zJõ?£ÃNʘ‰?êprÓÔuZ?­ØK†ì6Ø?¦Î'8$Êë?•¯*³.x?ÀŠªâÛñ?ªU'{ï¸Ö?ëòþR‰mZ?¬_Æùžóé?ƒ»I4®á?€'ψÎ?¾6£üÓ?¬»qç–AGN3FGL J2215.5+6122@ZV~ùÛ"Ñ@™l?Ä;.À9Ó'YáÀ:Ég¦†é?òíȀþç@
Q[ÅM§~@;¿Ý/ñ¿Ò±kã(þ¿çèFiµ•¿ë…ü~ ¨¿å'ph]¯UNASNone?À7(ɀo°?ºfšÖõ4?ÍasH³3Z?Ä"š´¡²Ã?ä™Øûs>?ȕÊ4ʕ™?Ù¾Öüæ?Ôb¾Ýz"?Åé½jÑ}?Á¾ô÷'-/?ÜiÌJN‹\?Е²Ñ4æ?ܽmúÅÈ?µbë¬&±?ƓšFgÃ^?«!>ÀºWÆ?×øÅÛä9G?µª'Ħ;?ÇáÉG!R?³_¶
·†f?Ô·#ߋÊ?Ã×["qï?ßWšYÄL?ÀG=°~|L?ÒJX;³èÙ?Æîw󽸙?ÃD:?p?¼f'!®"?â	ÓS';¸?ÉÒtn3[Ä?ääé´}å?ÔÕ
ÓlN?¼¶-0Or?Àü.uo~ú?ÎuÃP¢/?Ìó5nn??æj}e*C?°ÆÛØ>¬?¿îœ6VK?¢©ÈrÂa±?Æ^¼%,+Ï?«	~P_?ÕÀF"pú?³'ð¹Ù.?Ôl¦9˜°™?¶Œl
?ÕÓ(âÞm?²2­lÙHæMIXED3FGL J2217.2+6346@Z·#c²W@KpïVd'À92ÀÁ%ϝÀ:ïµk‡7—?ÙÒ
	ª^õ@
>>lLYu@v/ŸTïq¿ÁøÄË)<B¿èîaœýý¿å¨øál…Ô¿ãS'æ&]UNASNone?àÏežÈá
?ɬÏ0æ?¶q•§±/D?µ}øqõº?ØÄÏXÔh´?ÉÈ+ÝÿO+?ækµÂ]÷Ç?Ðö:áÊ­/?¬iVÄ}‹?°Ê†‡<K•?Ï6ÓCçéç?Ìs…U6_°?äÚgÝ*N?µÚ䂭??¸O¼ªæ?¢v™¶9?Ð7BÅUÞ?³t#ÁºÆ?àUÎ<¨@À?µæ‡†Ðê?®ä€ýÔG9?¡©°V·y?ÛwÓfš?µ™ŽCë‹V?é'!ËàFZ?Ä'ì.Ån?›Yêap"÷? 
áû>Aˆ?ÆL;'b|?ÂÛ≢€ž?ìkZñ,x?ÃÞ§œ!ðQ?ßlY
·?¨ó<†´?µ-M`[	'?½¸,#@ï+?ë³ýìæƒé?¥tnyËÂ
?§ßŸ½?"ï
@I?¶pˆˆûØ?¡Ê¨û؝?çÝø€.ä?¨UßkÇ	¦?§ßo.šÈ?á>Tì™Û?ʓØQ1Ã>?¦Š
ZËAAGN3FGL J2217.8+3207@V3RÒ4ëšÀ4_¢œwškÀ:Jß72œ4À;Æ|°TÇ¿ê©ù>a˜@¬Äĕ›³@(_o§-¿åØû)xí¿åÛr…¿®<¿æcY·_ü¿â*Ûì'þ*UNASNone?ï³ ™Øs?Î˜\3XÜ?_n†®¢ð¦?c [ïë)?~"PZ"?€MqÇFfÉ?îµ|î,Þ?­Ò•çòèÌ?†¼.'ZRS?˜0M?pP?òJöùe?¥·¢Š'E,?í@ÿ•¸Ë?œq0YÊÚ?'ˆ)ã?ˆ6¶´µé?­bDå)"a?–RÑR%c?íÆõi<ôA?›î§íÇ?s(§x.V×?pz"ë}â?°•Ê=a›?›oó·?ïåB4šU?'õ£õ®é?Nb¸2¸ß?€Pr…F¼?c%AÓ
?npÁà¾î?ï£a¤¾C{?}|eøô?jõ©³¨j?|É>Vã¡?€j,ŠÊ¹??†6jã2EÌ?福™W?ƒ§'–æº?‰¥ú¬Ä?w©³sY›×?'}œ°FÒ?wûi¼?ïŠQÒ}_?u¢JAë{?Q–Ò?Co3o¾1?‹8·¿dþ^?uTù¤~AGN3FGL J2220.6-6833@t»ƒÏ,ùÀE~s>»ýrÀ:p'Á—åÀ;úIŽ¿K?Á3ÎCoks@UQŽ&ô@
`V,?¼ôty­¹¿¿#H¼SÐ.¿ä­>!MØ{¿âiØd
NPUNASNone?ï÷ iyc?E'	n'©–?9ލkòB+?5ñn€±ê?F 7uf¤D?=L.ê+^?ï1¸K'×®?—†¥§î×?t`g'l?x†Ï^8¤?"Ã^u<~G?"É­ÛyÛ?îàFŠºô?ˆ§JW:|?•X¡"«A?€âNˆàùÿ?"aÖIžQ?}´K º¶?¨m¶¬?—ÓԍüÑ?‡Öp¼5î?~ÏEBjÚ? ÏYF§¶?•!ê+D‹Ò?ïû7J?7—{·§eÑ?*h 'Ä4?$³Øê?:25~'./?1§ê:'
‰?ïÁ±@²Ö4?z…#™Kæ¿?]ÜL¸eš¸?X8:¢öâ
?w°Li]7N?wQ¯¢Õå?ïs_›úzŽ?z¬´Tä"?'mNúu?u-Ó¶jœ–?€»»Uâþ?h1\	s@?ï²òÊÒœ?uØ
O¬a?i"z`fÅ£?U0Ž¿©?yõ]fãc?s&4"á™AGN3FGL J2223.3+0103@PMÔA5TvÀFL\|ؙÀ:>}—ÛSxÀ;­?)
»E?ÌÀ™~§â@
Ñìšó`à?üðxá=G3?ŗÊeÙ˜¿á½'œ¹Î¿¯"ç<Ü÷Š¿Þçg¾çB*UNASNone?ïÎÿ}+ØT?€ýjS¤Ð?9|(á¯qR?Bú5IJIÕ?vè~ÒkŽÄ?€9ÀØX4_?ï`îýE²ß?—¬¿È?nS¯#tqh?u31'DmŒ?ªk£çü?ŠuÕ¦,}v?îÀZÅb9?Š¨´r@—Ó?‰Sá‡!¥u?sÏ(û™Y?›J¶'ß×e?†9çŠñ¾§?í§•Ì
<Ý?¡#
oÒ?f…¾…^;±?kJË­£Ì?²#­…é÷? Ú"3?ï¸6=\_…?­wâÉ:%~?Eh½$oÛ§?vaYÓ?€›äÕ³¢n?«O"—fÔï?ïÍ)>›NÙ?s<ÿ¸¦ý?XT"f²Ç'?T(°àø?sV;ƒ^MÏ?p(?l?ïmwgF?zÉSï~?{t¯3]?aÜ£ýI"?†çâ^p\?w=́´ß?ïdÐj¢Fx?|"á,—?e]×%ˆ&2?VïË܎>?º7Âæ¤L?zMÇ®ÓYAGN3FGL J2224.4+0351@QšmÚÏÀEsG0@9¬À:sˆ¾€À;§¤&»U¬¿É'6G~ˆ‹@HtÓ¼€#?ù‡µ'm,?ïü6Ìq'¿àà~~ú˧¿áÿx÷žÄ?Ĩ0A\ŽUNASNone?ïåŒRÍò?f–Ñ?°u?3±eé$¨?-4Äu|sË?gýÉA?fK3Éç"?ï‡Æ³X1š?ŠJ£0mÇ?f)"µ¾1¹?sõ=]gÛ?ˆƒòzêî?…àîµj?î\ö;í'?'PwcO4å?ñ®6<Z­?€Y=˜mÈÑ?¡Åi}³d:?Œç7Lºœ?î8Å|T?£Ü®6¶c?Lù¥ò
;6?Z÷2 N?«ÿÁ§
ãŒ?£Ã–
Š?ïöbåÓY?JwÖ÷º?!^â?UØ8?
‡Ì.µ?QX>w¸]?IIXÃvpú?ïØÃÂ>~?mriþn)?RBDìö?PØ"Œ5?nŧÃ>¶?g¨k§?Šà?ï$¤à¨)ˆ?‰™•óÞ«?'YÔNJ·›?vl*",
>?'>y¡–6?†D²é?ï«%‰f5?{áXCé±Û?3ÑÉàg§Ÿ?8ÑÚX°:Â?"˜0Þ¦0Y?{•5š¨AGN3FGL J2228.5-1636@Ew}XÀK®ðà¨KäÀ:&êÓ²šÀ;¾Îf*…?ã'ó¬Nkã@<k›"€X@
Y ,Æ2¿ê£Oÿ'蹿äDn[¿å^gæ‡ø¡¿Ú·ï-}oJUNASNone?ïøGa¾`ù?G«[3êœ?7£5]ñ8«?7KZ2§ó?CÞìZ¬?@ÇàB¨'?ïm•šº®?'¼{ço?nŒ¿(@†?yœb·³G¯?Œ÷'hêòt?ŒMa•mÑD?î€bLÀë?•:XNGL?'Õþt›¥'?~9…BÏH?ž·õ
þ?†wà=@H?í×h"Ûw? 10cd?'ܼ˜El?"ÎþLÃõZ?­ÒO¼­z4?œ¾†P /Ê?ïôÆß?'t§át¾?7áíHèó?y2è'K¿`?P{'¸òœ`?–ÛþÁð?ïÐ;nëðÿ?w™Ços]ù?W÷õŒQ?_²cÁ?qä…bÄ]?q¨ÅmRA?ïqrìì¨?t_WõN'?~ÿFý~Ò?g©¬£?íL?"#×ÕzTŠ?kÞ¦ýyú­?ï|E"ùe¡?F&ÐXXk?sÑ~^v"?iz<—ïû?‡ۇàm?xæR]§7AGN3FGL J2229.1+2255@UB>ÕÀ=FژgjrÀ:9^>y¸SÀ;ÊPg÷`¿ÎnÝ	@Oðò'@é®@o±¿¿åüCà‡¿ãù!3¶¿és¤¦©M¿®µÎCõl6UNASNone?ï²½†+ÿ?|hGn?]܇7¾É"?aûÜz'?*Zá;Þl?"chêÙ?ïb<>ä[#?–FVÁü»Ý?rRئˆ&?€Ø¦—£‡?ŽGƒø±¼?Áe蚬?îË-ª!?•ÚÑýv(t?—Ä°gŸ(?…U"öÚ+?£ôï֒?†b+Ú~…?îòé½Q?•ï"D¹;¢?X/3–ÿº!?bEMq·Ð)? õj "Ñ?•§}íG"à?ïìU%¡OF?b\èÿ$?AÃ;P{?G3ðçÍЩ?^t¤Ue?^´AÞ'?ïϋD'ˆk?vJì쉡ñ?YM+Qqr˜?`oò25R	?qç4¼%…?pXqŠùš?ïD4È^©?}BËÔÄÒ?"Ü¥8ÝaÝ?o¦$[?Š(¹Ç1c?t¦ÃÿÃÌø?ïÔ—@Eb?knØ¡Q~å?5Ɲi É?5œJ6'ü?t J¦×ñŸ?j‹|aÛ«MAGN3FGL J2237.5-8326@s3"µÜÆ?À@DÈ`VíÀ9¥"L["fÀ;6dÃÎ÷?àŸñgêR¢@¾æåÒ­7@x4€3>¿çð¥ë>.¿â5v{Ô¯¿æûFf…‰Ü¿îVP.@°UNASNone?ë$³c͸c?¿žzû…D?Ž¤±¥)?¿L$Ӗaù?{ÑÍ
áå¡?x?4Àç†?í!g)œN?²bµ›Ô¥?œê¾v£?ÝŒ'¾ì·?¯t.,—P?­f›d{Ó×?èøÞ¬%ëÖ?°Jìgþ´)?ÃFZÄéöÌ?«*û¿õ?±¬UûA?šç&‡©?äÝ£…ð^;?±œ»(âk?¸Ç~юŸã?¡ÿ-P¨áw?ÐÙ?»›'?°ë{Ö?í;Ëù¼3?º…à÷t?´»´ó{¦?¸Êlÿ•s†?v_(b'p? +ڊ‹ÅØ?îå§gk&È?Ÿ_ð{^¸K?Š—mø߃?‹»kZÔÓP?–<Çb}ï1?—ßÐUZŠ?ì›a/ùJ?¢¤Lhøâ¶?³>Ïm)èË?ŸWý/$¸?Ÿ˜œL/9?+§
¶áU?êÝ{Þ?2g?žÁþ|B&Þ?­™ñöUpñ?3RpmÙÖ?ºG(GÿQ?˜õÜF9"AGN3FGL J2244.6+2503@Vpڐî¢À=ˆb¡µÇÎÀ:§x+ŠÈÀ;æ<³åu?éÉÇè?!²@
Õíðˆéž?þ¶1_žv"?Ü*Ž'?µO˜©
¤¿ÕQ:í^45¿à¢Ou´7UNASNone?ïðÙÜL>?Zñ9·~?6z _B?4‰ú8v?XÇ(üÙ?W éø^Mw?ît²†œß?©®ã›¯ï(?Œhý¾ˆñ"?ï9˜Ä?¡š˜&Ò??¦*6Î1÷€?îºwÜ@ÄR?[ìúd– ?ÚÜ;=?~mÍVîï?™Ã–U2·?"Æ¢.£?í#š¹Õ#?¦½ ø˜?£kÎÿ-Ò^?›&í¯ºP?¬÷PéXr? YŸ}!ì?ïô¼gFW ?_Cáýó¢°?-ö#Ù'_?5íãSêi?RÈlœ\«Ë?ZóáâÔ86?ï€õ#`µÖ?AŽÕb¡?sÆôML–?sŽ,Z©RJ?…߶uöS?Š0yœ^E?ïl›]?x¸ªè¶·1?Pú\|T?nã¹َÓ?…1:%}?p…okـ?îóLþ,ã…?‰>Àû YX?•$Œw(GË?‡‰Ëí&?ˆã§—W#?~3ƒ}ŸAGN3FGL J2247.2-0004@QÂÀð ÀHÞbäѦÀ9åóìÌÀ;›z6'?Ëøòd•x@	E—丧@Ü·àð?¿b v°¿æûÒp¥¿àÞ+ÿ7X¿à,_ÃEJÉUNASNone?ïï nVí?XÍÎjá¿0?;¶dϲXn?6M¢¿n*?Zъ4Ãth?VÍ8*?ï?V‰|ž?–‡&äì	p?rh%݊k?yÃ|g"ĵ?"{%œ9	¡?"ÅÒqLTŠ?îÅœ£ j?Œ¬ÙJ0;6?ÆˆÝV)O?|"HŸr Ø?˜|hH?";Çe1˜‹?ì@†o	<?¥,¶{Ž?}:ux}?x/iöÐî¦?¼øæŽÈc?¤ªé¬<4?ïù']´]?C{A"üŸ?-Åg'?'èÿÅ?D Ø$€si??7#™isc?ï¿|πÔ?{F²Ž¬"?]OÕ
HF?\ò)*?ÿ?wLLO]*?vó¨tûïî?ïB_Ëí?sÝåH{/?{̙ÖÀ=‹?iz…šB½¾?É2z—q?jÎx¼³ÞÂ?ï‹fŒ7?"b""®?pT1ÅÜ?Zо`°¿Z?™r¢'ëS?ƒv	"DõaAGN3FGL J2249.3-5943@tqŒ½D¦ÀI¥¶…ì>À:åwo£&
À<'Y
]QÀè>WÔ}E@
ŠÓÒO˜š@dhÀí_¿æ;Ïl—á¿ÖËÑǀ¿êêu'°"S?ÈKÕI%ÁcUNASNone?îÌLéßús?·¦ä¢—Ê+?Ÿ/Š,B,?·§¾©^ä?}bïÔÝ¿?|P±Yçðo?¦›?ˆ©G\lã?dzaºîõŠ?uë±'Ü L?"Ú@×[ò?'ELòî:Ù?í^aE{pu?›®,Žú?£;bl0Õ¶?"†aBµK?¦Þ‰=Ïðù?'Iÿä¿A?ïê5?ŸI©?hÍaÆj>êJ—¡ ª?%–ë勃?e°uÁ‰µé?hÆ®úx²f?îèNg¹o?ÃXE,$?¥"?5Ì ?©`'x#c?uB{)?¥Ö*[­¬Ÿ?ïÞÑ·m??k "7¼>?P+ŽÄÁu?Pcøßb™-?i#2ëªÕv?dþcmñž¶?îҀ"8V‰?ŽMÕå"Î?"ÓÿÆõw?Š0xÑt'©?ÛíÒt?|gú«Ÿ?ïý'KÁ–Û?46&2
>«ÙÂ˟Üä>³Ùe¹óe?3ß´,‹	Ï?40kaãSAGN3FGL J2250.3+1747@U–ª:э&ÀB*R¤ À95Õ"äFÀ:ë°Š`A¿×¡³†!9-@ݽ=¸@@H)`vP¿ê¹ý¯:7+¿æ~@–âÉÓ¿îìbïŽmÁ?á8¶ªCUNASNone?ïìú†»½Ó?mÅÀDMj?/ä"K7YÖ?9þóí?a1*M.?kÕäã|/?ï•Èÿ¿F?‰ 3À
—j?eq¡—µ1?u	gÓ½ó'?…1W§6U?'¨—!'±?ëËIóq¯Î?«'Ïž(î?£%øÔeé?–ið2O(?¸³ú??¦'Î6j†m?ïKçMB?–Í_',…?Nè
[iz?+Ž¹9D¶¾?–nÐ6FŠ"?–Êd/
Â?ïí	U
ÀÆ?‹V;S(?#Ì©'xÒ¯?J….ž;#s?a¹à¦fc9?ŠÁë1ǧ?ïÜԜ¤æÕ?kWR#Å?Qn¾Wž·c?PИ2¸ Z?jtr¢';?dãTkûC?î:ƒÿý™?›®­Xçmz?Ž |¸2B?†Lñþ¾+?¤Ï¹ëb}è?—êuÃë@š?ïßyžb½K?l¥Æ[k!>îm6Y"¼?À"Ó´—?p3ú.Šüü?lžÂWcÎ5AGN3FGL J2250.6+3308@WêÝëÙÀ7AÐúX÷À9ø8¢Þ¼¹À;Åß3מ?ó3¥^sÓ·@
êr$4¾@ÕãÿÄEë?ÜdR5¾)¿æ>k‹nó¿éΏ¿Q¿ïÿÙUNASNone?ر†Ô߯—?Ì$ð-Éa?Ӆ%ptS±?ÊùV^—¡-?ÓÉS»¾Ýv?DŽÀ4Ÿ*8?¿uE֒¸?»!ËþVîµ?ä¨&غtc?Å 7'[?ͤÁ±ÌÒg?Á4E¢e_?àîCPGý?´Ahw…?՚ýâ[?´!nÁ}#?ĎL¼ú¥V?§¢ÂÎvd?ÆÄS48ˆ?­;êâáY?æ9ù³,43?¶‡Hl×ùä?ÀSÅÿ­?¯Qû;ÚÒ?âuî§(!?Í	·¦?̸ÁýæË?ÇìÏÕ‡?Ê%ŒŸ"·5?ÃêZº"C¢?ÒÕh…X"?ÁÚâ0®•÷?á,Ï/Â?Ãåè°
Ó?ǂD{¸³?¹do'ïgh?å²dy&\‹?°ˆ'e?ͬqß&§Æ?¬Ü6¸}ÿB?·øuì?Ÿ¡@˜&ó?Ýâ–kDz6?°;PîBþ?Ýw
5ì~¡?¯ã‹/g"p?²™}{ª!? äÖ>F©áMIXED3FGL J2253.1-1237@K\bõ˜ñÀMb"aùðÀ:$tÎÀ;ÖËÒÑɌ?îy‡ôom@¥Ô/^@‰åÿά̿ØeöÕ¿èud¤«µ¿ç1ÉÓ7
ø¿ïÁRÿx¾UNASNone?î×÷¤?Ÿ›Ù't»?–´
W9Ic?™Yº0'ïÜ?ŒšhŠ‰Ú?ˆö˜"K.?碀"8V‰?ÃS«Aí?À$äPwÙ?·êhó:?ÁQ`Óˆ?¶Í:ðf»é?éNŽ'Ü‹(?¯e@à:ªÛ?Àñ¬lÒ]¨?¨O1¿¶Pï?³¨3œ¬ì?œ¦U@ƒ´?âÈAðÛ?³†ŒŒö²?ÐFD¿ÄóÝ?±Œ}‰¨Ô?Ç@Uv;]?­èa4Ŧà?ïÛçlf?žâ
}v`J?"òñ\u¸?š˜*ÄÿÂÑ?†± iš?'·),36§?ìaeð
³a?±%Ìhœù*?®êå±] ;?¦üj>:ý?ªþ»LÛ½? (‰¼ä?ìzB4ò"Ì?¢3Ė‡a?³`ר•Wb?œvPèp"\?¡š-_¬x?ŒáN›
áD?éÙñ·èº?¢‰>çg ?Á‰Û~žõ?›Ú"XZX=?¬F'äOd?•o¼U¥0ÎAGN3FGL J2254.1+6229@[v"8…
@ ݂ýuâÀ8ÈI°M:EÀ;Gckà#?ÜÉhÚ	 e@A⹞ß@}_Ò"¢¿áßZËuU¿éö¾á¿é#Y…ú¢À¿ç§2ŋKUNASNone?îTô¨Ç=?©«:¥Ê'Í?Ž°ëž2Ö?"8ŠE—#?£1ØwøJ"?¥õS–ºs?äӁ;Çâ?рP9u¹ã?±ÉQlT+?²¶E"è7•?Ñæ©."o2?̀€È+A;?è °*:ø5?°0ü³U"—?±öބŠ\È?Ÿb¿ýVc?āÐ"Ë?©]"3È?â¤HÞ/?²ØrlÍìY?µi¦Ò̝?¤¢aέö¾?Õ]­" û<?²Šã6ÈHl?ïÌ÷ȁ—?'Q¯…,?nb<ÔP]"?påu3·~8?ˆt2Ù{nÒ?ŽíI_" ?ë́\ÙAG?ÄM'X½?¡tw©¸S?§-y…³ûÉ?¹ºÜ…2¢?¾ÒèÛ L§?íx(u•†?ûf6lƒ?žÝ)ÿòÞ?Žè7B~®?©äx2?"'ÜÍ%+@?êDà`? ër™<·?¤ñôõ@ü?‰6s]Œ?ÁèÃ:VO?Ÿ	®—'	VAGN3FGL J2254.6+4253@YM†DR?hÀ."'›ØÀ9µr҅srÀ;"=?%¯½?àFqï0¤ã@ލz&@FHö…X¿æ]ÓèŸç¿ç`XUŠ(Á¿éèx'{M‡¿ïÿ–ȦCîUNASNone?[ÿ/K?Ž;ÌÓ»{?xç6¥l'S?}=Yâ%x?~ěeJ¬Q?‰íôrØ?åÏ ¼~?Ço6患?Ä'B G?¸T¸²ò,Ä?Ä£|UyÀ?ÁúÍ>'?ìG"îRó1?£o§ïÒô?¯û识Š?—h/Ðckp?«øµ2ý-h?•å¼Öâ.Ç?âó$­&"?²˜Þ>×Z?Î)|
 />?±öǤZB
?Æ	ó««6q?«a.hqy?ïˌÁwŒ²?yc3‰5Ê?f.aìFù-?fú);ð,?nDܖ¬ôÒ?sþ¡àÒ?ìÚHØ®O?¹zFDTe)?­ƒÒlzÐÌ?¤ìJßài?°oD"Fÿ¡?±¨}öX"õ?îclº¤'W?Ž7?hg÷?Ÿ±l˺'?"—S–VÎ?"ƒ·9zŽ?|ð$Þ6L²?ëZ¡€æã?ž%,!€Š'?¶cÊ…éœ?—¥íFM?­Ž¬Y#'?"X±7"¯AGN3FGL J2258.2-3645@8R÷ô˜ÄÀP$³=¯ŽÀ:¿Â"À;ïìì'(¿²œN˜lÝ@29Ÿˆñ×?ÿKA¿½ð'¿ãá•5¶C?Àe[é«f¿îÃnšµ?è«é‡ˆÊUNASNone?ïŸW°ãY¤?"˜þÐ;Rx?g#}­Ê™?m§ہfä?'a4æ΁?"·IáQg?ï'dõß%ü?–B¸(©V ?gJ`Äa~€?×M—(Y?…Ô*Vn5c?;Ú:^?íYB ¶ÙÆ?Ÿù:þ~­?ž•¥ ê?<عÅ'?«cN,Sˆ"?š•)âx?ïeJæ"ZQ?—=+¨‰Ó?][®(©5Ô?ww¸êàèœ?'€èPi'ƒ?–Y$ÈaX?ï×ÉEéi?x
]»»æ?L9êœ"?T'Ÿ‰y78?p™–&åøc?u{÷ìæë­?ïÜ(í´ùÇ?|7Où#?RÖ6½µ7o?i4‡
(É?jk÷/ƒô"?q«~±QjX?î¶È…ç?'kU¡b´Ø?ÓÃOå4f?ƒGœåg"?˜S<bèʳ?Š‹ôÞ-?ïî!¢"el?geÔ²²¨?E]'— '?3tqÆ¹?`ä2Ùîá±?f¶0Ð@ÃiAGN3FGL J2258.8+2437@W.~ùÛ"ÑÀ?­W¼xÀ:ÈB#'À;š‰;}"¿ñœÝø©Ê@¥n‰ }9@xO #¶é¿ä¶_ ˆÿ¿îŽ:üçX?ÌÕp'î¿çQù¶©UNASNone?ïøùzÎÂ?L'W·¦¦?e[ô?à4®i|Ÿ?Hú©Ï-—H?Kpù†/,?c "S?‰!f'–?iL™Øûüˆ?t X‰ÎY?‡>ň*?ƒ="	¢?î[võ;4?"¾ý0‹ÆÅ?†€ÉHp͗?sH§ YS'?¤¨^[ U?'BèAyE\?ïDøfìW?•{3Lꆠ?ŠDî\.?0i¡:å1Õ?—Dhó[X?•nL[DÁ?ïûqì4#Ò?F"D¸gmv?>œïö?+š­Ü?Þ?? õ·ˆ](?DòQ\Վ™?ï×nLŒ'?nôØ£%y®?T½¡,&Kß?RÜ
Ü€?n2ãMàè?h±3Ö|'?ï6hrT?Š*t콸E?u›´Ðy?bÐâsÂ?"ö5jN?‰ä6uÝÒ¯?ïÝvízË?gàýÅãÛy?ü½Ó	–ì?½gí¼Ç?q$ќC…Ï?g•¸Ò,¨AGN3FGL J2259.9-1553@IXÜìÀNëD$>ûÀ:O&ËEäÀ;ãpûÞ´?çrÝæƒ4Ü@&î'm¦!@å®À>•¿ÞÏ
Ž¿à>íÚ?¿â"%¸«¿è*‡= UNASNone?ïÐqâñ?p£ÍŠAùÔ?T0	q©E?Suç9Š†?rëuëzÉ?mPâE¯â†?îvQSb[H?£ÕßþªV?ŒE|m6ñ?G—8‰7?¡‰‹°RÉ?Äöwg«æ?î=$«°óR?'‰.÷Á?"g›¹'/?€ŠÄtåã?¢yçd¸\?‹">fã¦è?ë4)´-€?¨þLy"?©"§ßRl|?›Q(RÕ?¹Íc`!¨Ç?£¢Ïi³m˜?ïîÕy(
?Vÿ¹³¥?7òTéì–?3¼ŽYčÄ?\Y5!æ?T§Õœ×'?ݹÚ?†õMó»À?tå¼ûN
"?rΣr¨—x?…*ª
›ˆ‰?€çKc`¹ˆ?ï[:&¨œ}?xº_üƒ¸v?€',ù3cT?lÏ8ڋ€?ˆ IVÎ'r?pkŠ+)[é?îWÖ8
!?Ž÷ÅÈqÁ?_q_l?×Ap'Ñ7?—¦%éՎk?"×ïO4šAGN3FGL J2300.0+4053@YO‰ 'RTÀ1>%Øם
À:5D…kÀ;®ÖuÂú¼ÀøBÃIs@¹®@ð‹?ø9	Ü¿ïØfNq/Ì?îßë5v7¿ìÕ&sÃW?éV¸MäºTUNASNone?ïc/Z
¸k?šs‹¼,Í?jS
mu?q]
ǝɹ?O´¤?™·jj ?ïˆns¤ž?'˧|¾ê?lÈ%šW¨?t\¥`4è§?†àq37Ԝ?©np‹Œ?íPDPxl?"φè?¢û?2è,?•àéi"Œ?¨{Ï$"?"(ÈÉ}—?ïð_«ƒžR?iå;­…>óË(ä]›L?º(_扨?^ñ|¢oƒ?iáoF‹áê?ïI7¹L3Ø?°dcñ…Ø‹?S‡¨ªªuK?V_­smñ?• ŽPF[²?°a7ÛÙ?ïØ|±"y?r"½e?æ›?Tø«'vÆ?UñÊýþ"¹?mùcÄ£›?l€åø}¹Ä?îG±/‡ù?š—Õ1;?šÂÒ¢ú–_?'Ú°6ÕYW?œGxΐ?'>o[À`§?ïýà X?8[ûÐ>>'ÀýÔ>¢qôÙwç?0ûâÃû)?8Ø"vu*AGN3FGL J2300.1-3547@…Ø=CWnÀP66ŸÏ=ÀÀ:Iæ¯ÌâÀ;ðXr‡ÜÙ¿æ
zßwÓ@FEêE¾@z7?‡Ts?çh\eþÚ¿æpÙquä¿ãlŠ2¿â…f®'+`UNASNone?ïù*«Ð'ö?EPH·ò"{?ð˒×?	¥ÇFÁT?Gó3 O?C'` …‹…?ïj÷^‹?ŠÍׁ	>"?f¤ìô3'Ú?u*ƒ•Úõë?‡©ôõN»?…*Kjýóã?îâ~«¤?ˆÌ, ÁØ?‰øÞÌÊ5¨?wí!:<.?–¯àÀ»À?æ'Ɛh?î¬%ûg>þ?œ/¯½iÏÊ?V€ñK"?V÷FÀ¨*?¤‰FM:r?›Æj0c?ïü ¹ëÀû?0¬ô8‰ãn?H_»p˜?
¢$È!'¨?6(¿ŠW=?.•ŠßÎ"?ïÛŽÉ(u?mRFAKÝ?QÍ?!t¸?Qu/"ÄY?kýÑŹ–è?gwèÑÉ?ïƒsH]M?t薯"å£?{9¢1œpì?mÕe>Ÿ€??†\Õ]ßî?hÚõFK
y?ïÅD‹"?sÕéóx"?5v³I"öþ?-dQÎ> ?|rš¤Íÿ?s"!ñP"ŠAGN3FGL J2303.7+5555@[
…Æ}þÀÃ@&`¼ÙÀ:@»â™½¬À;œÜD9õ?è»[.ò(@
Z[k5®?ü‰Ÿ¦xû¿Ü1튩ß?ïû­9ÙH¿×þ}êªr¿ä
4Ô?>UNASNone?ï@U=C?™d§Ž=´°?hCp¡_'
?h²¢áFŠ?"ìê@Ôp*?—zL	^q§?֘ð0…?Жã~6‰ ?̱Þi§?À·¡2À?ÛO?Ì%%Ã"?ír'{H\?Üi~ÇüÆ?—"˜	üœ?…q¸"4e_?­'±.Fö?˜ì/Gÿ
¶?å8íçúz°?½uì<?ѧÞåÊÜ?¼k`@™p?¯20ž–I&?§Üµ,Bà?ïË÷́}™?w›N7ã÷'?M'\	Ö~?K¥ÑN?vSÍ«›¯?u Ù•I6?åœ6Ž—?Ï	Ɣñ¶‰?¼À[:ß?µÕð™dþM?Ë.úVV?Ç)LLV?ï"#ãßä?‰~­×ˆj?†EŽèV9I?uêò€Ô9?"J´Áàí?"7ǚó[¹?ëا©|»'?£ñð|7/­?»LCûWy¹?¡‹#·¤£a?—¹úߛ
Ò?Œü΍»@¾MIXED3FGL J2305.8+1658@Vqn?x»ÔÀC€¡UO¾À9Ø+{¯À;Aù¬ÿ§ë?҇‹-ŸÝ@´l8~L@3Œ¼¿éÌý°U®ï¿ì5 æO¿Úæ`æ¹vȿ纕KÅêõUNASNone?ïü•Ú?:Qïkr?
¸óÿØcÏ?6*NG£I?8(Q+Y«Ö?8é¡-Ó?ï`¥V]§?!"O\òe?o¢Ÿ"_ï?vXõÀ±Œ?î®y!?Š|÷×¥^m?îÂS=®{?ŽãõCŸ£/?ÿ?nòC˜$á?ží½SA¢?c=l;b?쏔]£&ê?ª†3Óo'Û?oñ05¨/–?o!ïZþ?ºƒÓ'Ai4?©øªk_?ïýÊ™W?0Ê,`ü?
½Â,žG?	šH"Àm?4)ø68Ò0?-ûNw\Œ¶?ïʇ¦ä&?sñ}5ÖÀ²?ZŠUš@|€?VÍOÿqº­?t—Õª	?pUdÎpAÛ?ªa?{fQ!i‰í?o`–ÄVIv?Se–£î Í?†º.½]?z¡ðyQ?îú\› §?Šj
}
…?nñ:"ÔF?[c+´ëû?œÖEMeY8?‰$I½6¢lAGN3FGL J2309.0+5428@[}VlôÀÚüGä› À:Ž¯à,üÀ;¯§Í9WÀ:$¾ü*@<9·[ÌZ?û('¿/«>?ïÿ/FOÖ¾¿áî$gà±S¿ê+ÛjjN?Î_É4
UNASNone?ï*u¢™?ƒ€"?vÞnãE?y€Øàíò?•9y½>?œO'm»?ívù•œx¶?Áês{Í«Å?ƒ×ä8o@?'v`Q4·?±Í6Ëi*?À¢€fwG?ìûY¸¶ê?ž¾P!?¡c¢™uñï?ûr@~=?®æÁޏËm?—'B¥q2*?ïwßæìÿ?"¢–S¥*?¾]èJš"?!mÂëO?ø£ìäb?"
Ñ«ˆùF?ï³¥¤>ä?"©Iؼp?]çšÎa?eˤâÚ¡"?~ÅëÍêU?'éjÂ5?ï4bZµ{?«¦†¨Uh?pÌÄ0GxÁ?é>W\"?•: Xbˆ?¨ŠõN«Ï?îxö€œ¿á?"«qýR¹?"Ô 
3ûÿ?…öÉñ1MX?ç[qÕ?ŽGJ¨€ùK?ïë×<ùkÍ?cUŒž'T–>Ãî»i¶"*>ÊÐ|f
?d#ǁ4?cTL"4AGN3FGL J2313.1+3935@YÃxFÜ]À3uº² À9úò03¤rÀ;º7'´yð¿îñØ@I·yS~@Xk 7™¿éD©Qü¿êÀ›ñ¸"‡¿æPü¸*†ð¿Ô¢[oéUNASNone?ïåT'…£:?x9¼lˆæ'??–|e‰1×?BœJ˃?f¸®*Gî«?vðß#X ?ïi³z–I-?'²ÌZ1ø?qãX¨'n?~¬v(ìÓ?Œ¡uIò×?+¨JB‹™?îr‡OÑP?a9¾®9?Ž˜ÝVé¹?zM@·jŽä?¡QäÚL̓?ŠÚ¢ÎK§ô?ï{xFÜ]?ƒž"f¾?/dçM¾2?2RðІB?R5Ã5"C?ƒ'ÓKÅdô?ïîÕ÷ªW?sÇûÖGnW?/Æ£Åê(?;Ì	æ!l?^[<¬6K?r§kþy—Ä?ïИïO®"?s6¶™ÞN²?XÑóÈz0?WP×±sÕ6?q"ܖot?n¬¸<q?ïeá8óE?}Ø&àÓ	?{ª'+æ^«?h$46–?ˆ²h«6»X?z8GmrŒI?ïë€`¯æ?X|äEÿ—?Ùè"Í¿?ì2W°©?dp9e@?X<ÃÅAAGN3FGL J2318.6-3829@vKÂã>ÿÀPáú~¶¿DÀ:Cê¡ô²À;úWâ?$Ù¿â"D‡»Ã@
Ò9u—‡@¡ß¹8›¿ã_'»Ëj¿áÑ)¨<l¿ásŠƒH–¿¿ïÿúw2šUNASNone?ìå>!''?Å3ú²§÷D?ªLZɨ?º®æe'Ä?²ª©ê~j?¾FÁEA?îIž¦ì	ö?§¥ +6Ã?¼ž2Xã^?"»yUeéè?£ÆxîÕë? sñ±ŒD?èώF?°/¼e?¹©Ÿì‹s?¢z–øi.?¿Ù눢^?«ÄóUæ@?í
|þêg?¥ØAñŽ?"\èð67?"yY]ãb?²ôÜÑ9?¡¡E0ö=?íÃ6dÚº?Ç~F±.$š?¦XÜUÄ@?½eE˜Õ=?§êð•¨?½Ó_"‡ó?ï…º'm?Šw<=7¯?uQÏG|Ɇ?yÁҐ`«Ö?"éϚ?2¿¼ä7{?ë–ÞE"Ò?¦çÜËè¡?±GüÒzÀù?›5ælel?²;Êó?¡.¿áûß¿?ï[©D:>?ƒ^L!"ÝÎ?o½ý¹?j0û¡Ô­?"%ÜÈõ?©²u'AGN3FGL J2321.3+5113@[7ÙÓEŒÒÀ"Yò™0À:ƒ¯'R£;À;Åú¬(©¿òSdvL7'@
XÕȞê¼@&ˆ "ä¿âm
&õbB¿ç¡˜Á'l¿ÇÏÿc-f¿áÅÐÚ#UNASNone?ï|FÌ[ýq?‹ÅNàÎA?@ž	d8[¿?>dwž8†?äl`,c×?‹iÉìIt%?îrâ?r(3?¯h¾³Ä
?©tW%?†!қ"C?¤Ü­y!3i?¬=ÖCPß,?î8sºóí‰?"À{¥Q"?à\ô
2·?xäB©\(?¥­½Ú¾?"¹ÚÉ?ïXZ® ï?…#)Á=¤?)u»'³
?0C"*9—?"ÁÀ"Oz?"üGÔèæ?ïÒ/îýq?qú'ªªè?74¾X1£{?5}$dBøü?u€œ4	
*?q‡£
?ï{Xeò£ ?–nUÐ"4?hðâIluÁ?o¶@mHC?Ší­ã• ˜?"wˆ¼ko?ïMéÑÚ¦?}—ªuÔï?~[¥lßoó?f¾Ï˜3?W¸ÕrXz?xzNo` S?ïÞ´¦xz?[µ%'-?:©¹íŸ?†`T°­?p=9¾ïÀ?[&@;CuAGN3FGL J2321.6-1619@KßÕÃÀP¤yèQÀ:Óe
 ÒsÀ;ÕSV¿)v¿;oX» …@
H€´ãw?ø†D 
é¿ïÿG+À^?ïÜèêi?à_ÝKRÂM¿âI:0¨iUNASNone?ïìAZ¤w?aµfåÎa´?)YT&Ü?%\'Éú?b-À1ñ?aVp@¯?ïA>þ\U°?£iÙ²jI@?w'Ì£ãœ?Šöñ<ˆÍ?'ûÃ\?›G€gÜl¯?î~xeSc?'¼åôÈÁ?'&uÅ'?ˆå=	Šh/?ž
†çq[?ˆæ]E,?ïjöoͽ?™á•±­Œ–?bïþz£Åü?~Š¿kx9œ?C2E&Ğ?—ܧxcð¿?ïôŸ|\œä?Sù.Þ@?!'k´9<_?
Êüù,?TœìÇ<?S."S"l?ï¿B¿(…–?…+ŽÉèß?d±Äx2sG?x»õN?v¾(ÄÃ2?vKýá¾1?ï#×gý¸?Ž*6ki3?‡ê6Å,þ?…f7<?US`Ӕ?"ôôz?ïÖsÖ!Æ`?sÄY:ç,?ZX~Œ¶?_|U²­E'?l_êÜ
b?o:
}LÁAGN3FGL J2323.7+2523@XÇP%"õÀ@²õýG¾ÛÀ:{—)|ÑÀ;â%™È"¿å=äiÌwg@gGPvÿ@__¶ôÉ¿è?+~UgÞ¿Ü«'GËú¿Þ"ZT®ä¿â1@1ôDUNASNone?ïø}Û?D'Š/³?"B˜¢Ë¾¯?±6êij?I8äÄ3T­?Cu,8nÕ?ï}ÖøtÆQ?ŠŸ¯ñpb?i§¼¬uÆ?tªÝFì?Š RµùYo?…‡ÜTj•"?ïԃ`®R?"7ìJ'€Ì?"ˆ[ÞÁúˆ?p·Øwd‹Q?'A¡œˆ?~ô©^UoL?ï{Ïì^Yõ?}víÿÿ¤?C…'±%'R?ASc~¦`i?Ó«ÏQ?|¿MªM1?ïü{k†5å?6£p—O?§0ðlyü?¦è]
Š'?7:Öcg‡€?5–V‹Ý?ïÕÔ_@?nQ»s…÷?TwËÄ´,q?Q#š½œµX?oðދùä?hØ;H‰e?ïš&s¼L?p"ØDŒ»R?u¡KGÃc?g‰|U¼ü?}Kla"s?dA˜»ú?ïåí¬ãš¼?V£Ÿ"Ú??-ÌMfƒÎ?®	­2)?h5'2sü?UÚ­åºZAGN3FGL J2327.2-4130@uºü"µÜÆÀP㦠YŸÀ:LÚ")=À;¬sWæpã?Áa^68˜š@µîŒ:5†@4Ý ·0¿ä¬ÍlÍ¿äºà恡"¿ë1pΧËê¿àØ-ÚóoéUNASNone?ïuá{ÖK?‹¥Ó	m`?x8óÅU?~p¢Íppá?†kD‹d?ƒxl_'€?îØ[êȜx?¬÷‹¾ëR?…o[R'?š…±uÒkÒ?š<ÿ§ÁÖ?£
)Ÿl´?ìµß*G|@? ]×[ýôæ?¢yäî7ÈÈ?ŽVU^[t?±7-?™ö'‡Ëg§?èPN±Ùä?µt<y¬4?¢§ çmlR? kÎ`Cä;?ÊÝ‹0Ü?´k7õ¼dˆ?ïØ–0?qf¬5>W?W†AGA?^Ž1O'	i?lv'+œ?iY¶yQ?ï°À ZØ-?Œ»:lý;?hë%W]Î?}0W}–·?{*c.º.æ?¢ø®)Ú?îÃm¹¨?Œ%Qþba˜?'+UüÞMÙ?°ޗÀž?–fòÌg?'n®H;?íÐl6i?—{€¨&½>?‰"ÏJ¢Þ?{¥¡÷i_?¬"t­Ü.°?•†qqýáQAGN3FGL J2329.8+6102@\M¶°_¯¿Òê~8•À9®ç¸5À;D
ð
­¿ç²9´¾@
:EÌ@|y ç¿è`ÎۚƿålMPjх¿ÇR!ïدH¿â¯3ŒUNASNone?íåî§ñ?¬a®_"'S?jlÌ-Å?fó˝?°ú)Š£?«Õ"Œ"AÊ?ÇŸwª£?ÑûS«´à?©æ-äó<×?¦Wó4?è¡uDú?ÑyôÊå?ì<µVIÉß?£qh–û?œä'Þ‹Þg?‰O'fz?¶á0–¹p? €£PL?ídÍZCöØ?¤¥›zWO–?Q{'åݒ?SЮÒÇõ?´"¨'%Ÿ?¤'êÆÚZÚ?ïq…Ÿhå?ÛtÃY-?^d%«ú†ý?b<I÷¸»J?Ò¾»Ð?‹çˆ§O?Ò֌4'j?Ös,)vx?°œW7Ý-?¦º¨f)n?ä)»É?Ô½¿€UrE?îÄŽöé?"û҇Ü?ŒÇÜkØ?~(ox›¹? ±óæ=Íp?–§F·f¸?ï;V©k/	?ƒªÙ…áaŸ?Ko¥Ò©Ý??"‡¿Q?—¹±í|?ƒLBk¼éäMIXED3FGL J2331.9-1609@MÒR'ƒÓ_ÀQ$GÃ
0jÀ:5õáõSÀ;ç"6Æf?íEförý<@%Ƃýk@SÐ@Ô?éãÁ^¥…¿àK¯"dP¿Þ¥Y¨ŠD´¿ïôÃaû-ïUNASNone?ítCd6hû?±"Aîu£?°Ï´…C¦g?¯ûY7ŠÍý?Œq'Ï'Åí?•M´c«hR?è*CÄêš?Æ©ísOFÔ?¾›Îò°¦?¼ƒ…ú!ë?À	d"Ü?©?¸‰Û##\?æ·äkO?³·þ=â?Ç¥n;X?®ud±?¼ŽŸÉ4?¨÷Oå}?æ4ý	'?½q‰KO?ÄèDd*n`?¶"MYúó&?Ãç§]kZ?³21ª—?íÍî'gÂ?²õüš¨‰ã?«•Ót-dÂ?°mê§×?Ž-(@ᨙ?˜,OÄWk?ë2SΏ.?¿Žœ>Ô?ø?¶=ârÀ*Â?¶Lº¯$ó?°/MšN?¨´ß'2X?ê^ñ'í8[?«ºFYÎ?½x*U‹o,?¤¬ožÄ1æ?¯ "%9´ý? *àúhG?ì:ðfÚÕ?¤8ü#—?³"'	ó?œ÷Ý€a*?¥64ãj%Á?™B°ÏwAGN3FGL J2333.0-5525@tC"Ðå`BÀM,k΅3±À9Ñï<c]À;ë›
ß½?í·&ÑaBK@
ð»äó	M@Åh`'6¿ÝèTZÓ¾·¿âïM,¿áéBËùày¿ïÿá_¥UNASNone?ÝU8†">?ËÍÀ/ãûñ?Ç%­:ؐr?ÂIöG‰ER?×ðÜy´?͈µVõ–?ÕÎEw®?όÜò´½â?ÜIï½Û©?˲˜×Zwù?Í.…×ùYP?ÁaÒDf?âtý먰
?·L'ÎÖ±?νyó‹þP?²DE
hg1?ÇnŽ]ÑA|?±:ú¹Û]¨?Þw´v-Œ?¼BOŽf=T?×?½ë2"{?½‰ú?đ=?ò?°á'-Å ?ã)y©—Ç?Ë*i{1¾?¼á¤0‡˜?¹T{yRdA?Ñ¿4£ ®Œ?ÉÜc+&'?àUF>0oè?Ï6
'Sƕ?Ö,¯Bg?Ê04ñNab?ÂQbÖ}?´8wœ—ñf?éˆcì?¬tži`b?¾ä«Mm"?£Ÿ4·bop?´Û%t9Ž? ù"uL³?èŸÌIÖI?­(رõj'?È[ÉIµ€«?©^©"ÊŽ?¬¦ÞhÃ?™Ö'+7҄MIXED3FGL J2334.4-7948@s1³g ù	ÀBX—{žÀ:OŽR=ºvÀ;ÃÍ¡Þâ?Çâ|_T¬Þ@ºý¡Uü@ø¨™Mn¿è›Ñ¯à'â¿ìitònƒ¿Ð½TÁMh¿æ
åH UUNASNone?ïëÚü\Ôº?aÕE‰z|C?(FzëSLÞ?+jèÓnU?b ›ÈžA?a\š¶&Z?îžn'>g€?¨Ö¼¹¹n?†ˆ	&ÙÙ\?'ôC3[w? wŸÏ\­?¢\š|ñØ?íñ!É\?˜Öuñ]u³?"À¹?½ŠY?¥!v?­€'ECHX?"÷.Ή5T?ìh–þoî?¬¸ü§¯&·?‰òÕË?Œ•û¼qÇ?»ÒÛ^:Ñ?ªÔ(ÆÞx?ïõ7ߌºZ?PÁYžyIº?  Sf¸s­?#2Áx!Ñ?SŒ6h3Ÿ?Pj*²9?âÿi,?'‡[ú2ÓÀ?r-Ë0êªk?)¦	œ
v?ƒÁ¡™ñïÎ?‡I¥?´Î?ïkN5K?ƒ‰õ,t?ƒ‹ïŸ!#T?só	/P;?"VzÅtçÿ?}o²êŸWá?îò¸ùJ?ŒŠ§j7?ƒ»ŽÜ4?tè ÛÚÁ3?—ËÓˆœ?‡EæèL!AGN3FGL J2335.6-2342@DW´ÀR#¶þ.n¨À:PJ›.ÅÀ;Ø*>—ëD¿ñ#†TÃPÍ@×8Ëùh6@-à_PÈ¿åÍ¹¿èy1ÈÇ¿éwíÒ"nŒ¿ß#<*R¹áUNASNone?ï³ûܞ•Ç?'`
¥!ù?aÁx±Ș?h0àα†O?}!UmvLL?IBCeh6?ï#ÌV
€?®otx•?} [‹@-?—[Ý÷A•w?"^Unô	?¤y1
¸5~?ìø¿è?Ÿ›‰Š(?ž^E*y?ŠOt²Y"?°¨¶«8?™¨¯ïÃÞ?ìÿ!	~È¢?ªù	aoà?mìÍWf
L?sróWÈX?·'J5p_?ª'ÂVOŸ?ïßè˟À?q4ÆMÝ#¡?MœbãD¹Ù?Väšêi¥?iþKÞ}?lL¬dÐ?ïƚFpZd?ŽÍS>ó.+?`N"þIZ‰?z¦ïxQ?t‹'Rüô×?"eý¾¼Ó­?îÝû
¢Æ>?ˆ:Ô±*t?Ž)µMW¶E?€F'L­u?•+ÄC?'E¦?ïnA:¡«P?''••Ù¾ž?@²ÇÌûé°?:]"=}0?'²Bhøjt?'Nm¢K,AGN3FGL J2337.2-8425@s}ŠüÀ@3EbàŸèÀ:v"Z»7À;¬1u¿¾ÚS"´,@
C˜LgŒ¬@ ­`uᄿÔΣUt¿æ;º{ïî¿èì|•å…?ÏwžëUNASNone?ï ßò)?"°Iü{Ь?`7-ºŠ—T?bõ8LµC?ƒºskú?ƒEôù‹š?ï;
©z¦ÿ?¥sç2¦1?xR

Eõð?'Ü{remÛ?'‰ÈQy*Ÿ?œ"ºNÉPf?íMcŒÂF?œ½é~óÌ?¡©Vö½Ô:?ê¿¿ì?©†rÑQîj?"gˆ?ù?í.θ<ûg?¯©I	ë-Ž?m°™Už†?€¹¨Ã±,Í?µœtR&?¯PñllÏ?ïݐ,;$ø?pß@vŒ?I™W5?P·<)jtJ?kÿNÝ?kô°øàñ?ïÀ¨õIV?3O6Ð?c{SùsE?-µó|ñç?uíÛn/ó`?pø1rÈX?îÍ3™¬Ü9?ŽjÓ|ú?"CCn?†¤œÔwì?"S‹ˆØØÔ?'b%‰.ké?ïK2¿?…&¦²Ü¶¥?J"Íáa€#?Tc*h|ŸÈ?Ž"æ}N¿"?"¾G–ÝAGN3FGL J2337.5+4108@[ÓØYÈÉÀ3ž¢	ª£­À:eÉÞÜÀ;Д9ˆŠ?Å+á×¢@@&Ít<"@ÎçßwÊ<¿Ý!.üö=è¿ìÈöÑ$—±?ÙJ»	ÖÃq¿í–©C'ŒUNASNone?ïvUÀ·üÂ?‹«R"´A?u\¯zvÔ¡?wi¶Ì2²?‡¼8ÿ3?"å>™â¢?ëUF±Ïè?Ä>ÏúåË?±Ág(Ï?»2!û¨Wx?³"¶
{ô?³²"!ÁŽ?ê÷"D^ºÝ?¥•>Vï.?µo–tdñ?Ÿ%tÖ,!?²×ÛH»…¨?™è§þõœ?ì²
ì|Àp?¶">Çôb?‰µ*-uåý?ó'CT­E?·8ëX#
¾?´°i¾`?sDV'?†‡j@Ê3?qþ±ã·Ì?xے¢Vo	?ƒÑÊ5äU?€7î ³qŽ?ìþUè·0{?Á§ˆÃ³t?ªñœª?¸'Äá‰?¥)̑•I?ªr¬Zx?ìÁqúÄ+é? KiÅGq?¯3Ub ?˜ZƄa?¤Ë¬ÿ6ˆQ?'üÈö¥ú€?ï
å+›íº?—Ê­ûU•?‡=0¾âõ?"¨â¼í?'Á»õÚ¥7?Œ‡1±NAGN3FGL J2338.7+0251@VsI''>ÀK¢±Ä2ÊXÀ:)>ku™àÀ;Çöåv?â#Œò
Æ_@ÛNšÂ¹y@¡u`F²¿ãÜ©""#2¿çuiÛa²¿êÿw(«¿î.'7$¯UNASNone?ïÍ2¨TÈ?q×éwÞ¡÷?nˆŒÎz?kpVÒ¼$Z?d¹Ï ¼qŒ?bkïc¿@?íß¼¢¡ïÃ?ªgÉÀ¥ý?•6Æl‰¶»?•±ÊOàa+?§hҞÀAq?£¸€Õ÷o˜?í"…#üñ?˜D'æÏ­R?¤›'´áø?urÑ?¢3¯üNÈû?‹¤°z»ðÍ?è`›Sá‡?­—>ϸS]?¹[N0¬ÉŒ?¢ñ*ŽÄµn?ÁLÖzÿ]?¨·­/ñÍ?ïÙ§¸Zà?jchÉ^+?gd§n¡LÜ?d~Ëò< ?]ç@! g(?W¨†I˜=ç?ïYû,—ÉÇ?î"䯸,?|¦ÇºGCË?|÷"Î'?‹-ÐøÊdd?‡
!$´9?îªÁ é{ü?‹êÌ^ŠFb?špL$c.?"±ÍV°F÷?7·Ž9N?yéÿŒ4zµ?íňy¥w7?'þÍ©UI??¢	_›¹1ú?ƒ1!ÊMì?¡žÉïZ"?Œ¦3ëEÜúAGN3FGL J2340.7+3847@[	H˒:À6	zû]À:Ž§©&ÕWÀ;Ô¡¹"ËÝ?°áȚS¡ê@
µp%¬âÍ?þ³ŽÀL¶½¿ë>¿0,¶¿í‡¶	U®?ÞXä¾í!g¿ÜB"Š;,ÒUNASNone?ïîL@lÏ?\+Rþýd?,•lm^?"âo†?a[??[Ù-æꛚ?ïq#ùPÛ²?'!áCÆ/?q|°(¦6?~2È"ÕÓ?Šø T¶a?ŠÜÁ¢ÒFl?îŠg="?00™ÁV?ƒµV"u?l¡ Pm?¢l6ˆGú¥?X˜p=Ö?ïL´¨á¯?™¯<g;?7Dìƪ&?T9.«×7I?–W5ÍÀˆ?˜ÍÍËê?ïõ'cøÖt?Mú·2Þ²?@%‹´‹?§"æÙ@?S·5fS®?Mnå}ñp?ïÐ%¦úø|?sj'	ä?Y×±6]Ó?W'L|,A?qwi÷Ç?n æë3 ³?ïU"Õ©%?ôWÚ¢Bt?v£¿âxÈ?YÃiq<¿?ej™Ðð?~›
+(×ø?ïá©Fú&?j"ÇÐh'§?=/faö?Gyçkbˆ†?jµµ-o·	?gªèh¸õAGN3FGL J2343.0-4748@t³Ý)4­ÀPY6z—À9áB-¡úÀ;Ü÷'þL?äzZ3I¥Þ@
%}$p@HVßà¥È¿×°֜•‰¿á$ÂÛ:Š¿ãDvcMq¿æç×FÅ®˜UNASNone@?ï'_ ap?"í¥ZNq?pÖs¥^Š?rn¸dsé¥?–Þ•òÒU?'Þ`Ó<n?이·¾Xý?¸ûñVp¯S?¤z.Pg¤é?ª—YÎ?°ÕCµL£?®¼mL<L??í[Ð7‡Î
?œBz#À9?ŸP´"sÆ
?‹j|©&ˆ?ªš¢C'n5?"U3–¸ò-?ç+üÉ¥â?²-àøx®/?º_—]\Û?¦†¬R¿ü–?Æ A*º
J?®%'Õ<?ﳬØe²6? ªßÕy?V¤+Wò?rp'[\E?€@Dy¿r?œ¤ÕéªHÖ?ï­NàÁT?›¿½'µ·?ˆê,Ë(ø?Ž3oHV=Ì?'õH£	?ŒQë+Èá?ï"–ò§›?ƒOsã	?ˆ´¶Å=P1?{®tází?Ž¥ŒÇ8þ?u"ã[ùí?íVÇx¶?™MI¥^ ?¨ڐ†É?‹ÂŽoë?§1ÄÝÛÒ?'À/B~MåAGN3FGL J2344.9-5647@t¶®}VmÀM/]»œúÀ:éÊ3•YÀ;÷ÂÅ+?Ç<;±'@W½þ¨¼ø@'3ÀvÓ¿â·Î?ŠüÀ¿êOüÁ¥8¿é'Þ¸©÷'¿ïÿååè=UNASNone?ïØY¹7wC?˜}¨ëÓ?6Íá²!C?9Î#µ`?rfE7L\w?—øUÑ=«Ï?î'f;À—Ø?¡"	I'·?‰<ÉɇÿÛ?‰»¾o'gû? šiє'?šÌThé?ío½FêAŸ?ž¸£}§?¡Ž×ƒ8´?Ö™¨}Ð?§uT´"X?—ˆÎå#û?ì¡	ŽZ\~?§ƒAìÉb?¢U8S"ü?"Tþ)ÔW?±Í‡ßq?£©¹?ïà"E9'?ˆà¦`‹âË?8eèÿë?Aˆÿ¥ôÉ?lYO&@u?ˆ@pË~Ÿì?¼þ£Š?"B¿à‡?s"V¾_?o Áün5ø?"UeV(Ó?~ˆŠÅl¹m?•?'P‹4†Wc?—xu\£o?"ºñëÛ©á?–U'r=G?‹y"ÊGq?ïG5ÓÃÙV?†gËûn?'Þk"Ëq'?rÆrÒ?‹TËo?'¥>Õ\1AGN3FGL J2351.9-7601@s9ÈýŸÓoÀDFÂß
A1À:N2 ä|À;­.ƒ¡	пۗA¹øx'@š÷0£‹á?û›A9†4¿ïÿ⿹z?ïþÌì­<å¿Ñ	Bsíã¿ÜS.¡UNASNone?ïãú ¼ñ?—"þ"Sh½?2¥€ßm?9¥*jÔÑï?j™U\™ù?— møtÅ?ï7ŠI*Òx?"¤Å¦'ˆ?uÔnXځ?{Wz&~?"ÊÃb?'"JZŸ¼Q?ît#_Dwî?'ñëåøµ?‰ª.lmõ#?w{±f‰?¢S>tŸÔ?NŸ:ç^S?îðò ¾Hr?˜?¨'£
Þ?}¨}9 
{?€zZr'ó¦?šwŒ Ú"?–ƒÉ?ýۈ?ïáÐ['e?˜‹¨-¡?#~Ùû
¯%?!Ôò韟?l÷·2â/?˜/Aïå?ïÄ{<ŒMV?xìª~á?]«ŽQÕF?Z¦—:»?vW óу¡?t­U§ì"?ïBÉL·?'í³$lµM?~51°òg?mL+?/~?•YAZ€?10S?ï·¦ê©Æ?t]†T€¨a?`ŠÓ³?UÝ
æU?|igí÷R?rº˜[šÊ5AGN3FGL J2354.0+2722@Zär\=îxÀ@ãÈ}²³FÀ:«ks¡RÀ;þ¢$'–H?Á{µÚv@
œ&"iY
@=ÿg©²¿ìs_ôx¿ÔŠÜŽG׿ǭ€'ú•¿é°6¿UNASNone?ïȇ#(Ù?v'ù©…
0?i¼£¿Uª?kMZxí$?m¼95¼‰?ke^…o¶´?î¸Bí÷{?žE<­×Õo?…<Ï9ÄP?…Z¾ˆ('w?žY:¡ ï?˜?,ÜD˜?íÙ[Ðؗ~?š"ÞY? ¿1¼b1Ô?"AÒ肦?¡«:_ÙL?Š ÞµÂ?î´dxöP?–Íj~}æ?»åBC*?½¢-y? Jø<`Z=?'ô7ÃèVÿ?ïݹ\~0?m¨Ù²×?]5H>æ£@?`®ûš?c¬HpЮI?b,g
i˜Ë?ï–CžâÀ?ƒ'³ Ü?p(Ãm¨z?jüÏ\,?'ZÖ£'×?|îWó|§?Vs?‡ªlüô?†N‰Ç?ƒ.Y8;Â?Š·È'x?uLU&ü?ï¡,՘oÅ?u˜{"ü?uuޒË?eɪLÔøË?yó¶Â³'?lU'Ì%~AGN3FGL J2354.4-6612@s}¼¾aÐÀH÷'·þ	À:?ïXzÀ<»Üº€š?؆èrÖÈ_@"Ú§
@€å¿ŒóC¿àSžˆÛ¿âæoÇIfb¿èGÇûèÕ¿æ†P´@~UNASNone?ï3x(–Þ:?—€-»(?éåSWÉ?ˆ˜ûË#;?œ<m!I?X­—Ý"·?îpR0…?°Î홧Û?½íùқA?™æOË?§ÞÈ'?©>‡õ¯?í<Il…L?œAÓg¤1¬?¡Ó‡ˆ_c?yŠ˜e`.?ªgá«J(ë?'Îvnfýõ?ë_áp·'ì?ª³Ò§Ñ?«_\1ß?#?Hd¡(ÿà?·QFaSÑ?¥¿Âöz¿;?ïÐä2ˆØ?vÎ7"µ7?Xÿýœ½?^½ågj¡?qŠ&ÇÛo?rŒío9^?ï…òï\ï?·Liz?q¨¸¨Íóú?v¾š}lÙÇ?…®çÜ.A?ˆX= o?ïˆ'¦m?ƒ%ßÎâD¼?ŒÅä§ê'?z^ÁâOX?Ïà
² ?uDí:'ì?îíçˆ\R?‹Õì',@d?Ãä¾'?wx®ÃœW?'×Áݓÿ?"¯ƒ™Z¸AGN3FGL J2354.8-5245@tº^5?}ÀO#ˆDÀÀ:åw¾}À;¡7qÁ
?ó!–é$e@q"T[!@C}ßÔ¼Z¿è¯S´KæL¿áòUÎÈ¿æQێþØZ¿ïÿóì)$UNASNone?ãaH2&vj?Ðâ	äŸ?Ô×B¯Û'ü?Î "Eô?±˜³®ðMB?³ƒ€–=?皪<Ó?Ɠ¢+/ûé?À¦IØ]œ
?½í
g¥3?Àï
Ò¯Ž?¸+a"Ì¥W?á¢rjD†1?¶-ÉnvÝ?Ó^¹&…X?³](ï]?Ã?xä Ü?©ši)ÂÐ?á¡ú5]&n?¶Ìª†œ~á?Ñ(è
'\0?·)Eì?Ç&Gf­è?­bÜG'å<?è!¦cµÉ?̓j.á® ?ÇSSº^L?ǒŻœ´è?°L%pZŽŸ?¶ûŸy%²v?ëqÖßȼ?»ÃN7µ?´ì·%®Ç?³-Š‡ø?¯	$l/·?¥ŒR~±?èÂ#Y)?°%VÜZ´W?ōªœä?ª"ÅÇú?³þ™®<hç? Ï"lk?çÆØVM?¨IÝ\¦™é?Èê­%›"¹?¦?¢x؇U?¯çÆ7C?•PÍ¡(Ç.AGN3FGL J2355.4+6939@]"_®¼@Ž@<œaÊö3À9±a8)<9À;)L$›À»?Ëý5U@
Ò	ÿ2O³@[á ŽÂ?Å%£'·Ôî¿éÞm^°Ã
¿ëšMbx4¿ØôMyÁžUNASNone?í:õä^?¸b¢¨B9?˜¡/~âwô? *®!¸wÛ?°žE
?´Bhg>õÖ?ìxÀBr7Í?ÂDÔÕH¶?"èÞr«? ÜG"7`Ý?¶ÿüsJm?¾ËÛ¤ð©?é§Y%5C¯?¯
·øó?°Wª0™f?›VB…JR?Á6ÆZí·S?©\+YQq?ç'Äs¤Š?µÄ6x:ë?œœ–È¢Ô?œRèÔA°?Îa_ºêeÿ?µFQwZÄ6?î¤îRó0Ó?¸!&µ.G'?'?Zz"p?•l°A ½­?¡!Yx䏯?´Êí¾MÇÎ?îø'§S…R?©t&ÐEʇ?ä¯(ä["?Œg_›Ø?˜öQ-"ð?£`s
aê
?íÆ÷­?™Ék%¡?ž7óõ L(?Qý¨Ö±$?¤t‹1ëÃ/?'M†׃?íN'õ\?šÜü!'?††âW°?y"ÂZ'º?²ÇÐ1>¯?™‡ìZøUAGN3FGL J2356.9+6812@]yèPð@'ó!Ë+ãÀ9oÑI3PÀ:ÌÀˆì?ӍŠÛCe¹@âŒQ²z;@
Aߞ`©¿ç÷݆S¿ëš{8Qøh¿çì"2Á¿ä:Ä—UNASNone?ëÆØpç@8?¾
	ÛÝ?‰%Ñ˺(?ˆwí;Fþ?¾¦·¾Œ†û?½Z±ý=­à?êØ8Φõ?Æ
~Fç=?¬ô¦kË;?¤2ރìO?Àé÷êÄ?œ,ªò¡7?äΐá{?¸ëÅSQË?µ$þú1Š?¡GPðŠ "?Ñ‹VµÄH?¶9ÞÅU?â»P?¸d­€0?¡ž3Óî+?•À
îøh(?ÙÈÂÿ
a?·µ·éX!>?í¬dXÞØ,?·Yn²ðk?q¤£¾®¢z?tdxjȌ?±''þ:8?¶ª '¥A^?îX1§9aÃ?³w°ãߤ?‰ä^`sãF?–¾êSI?¤Íñ¹6?­kÙLåf?ë|;*V?ª·3z¯2X?¤ÌEÅ/j>?"Fò4\L?¹¹{C9²÷?¦Ôœsðeú?èþtâÕø›?©4ó¦Ñ®?šª5ɨê?ƒg¸´Þ?Ȱ廆(y?§áþ§Ú1âAGN3FGL J2358.5+3827@[ëúÁҝÇÀ7BŒG¡AÀ:0/(âwYÀ;¹‰Úõr¿ØŠ$¾@¨ZéZ¢
@Ÿ?Àà?ïӇ¶–¿âØem~¿â"'«ìW'¿ØÐÁ'°ÁUNASNone?ïù˜·"Ìó?=Ñm/(B²?$Éï?®áþ*ô?DußOÌѦ?9¶£ªVÈ?ïRR,ó~?œÏ#¿!é_?sÒt›ÊU?¢9y[?Á4‡(û7?–èÁÉ?ï<–D‹±?…xêÔHõ?‡ꡆéb?t9š‡Ø?"ªwëÒ?€î`± Àb?î¡Còs$?šËJ{*A?[،ŠC»™?[š|¦˜Rk?¥ürß)?™À»0ûÈ?ïüÙÆõI?0É^g´žŒ?uÓ°:^?
¹¸þǶ?3Ԁvãê?.D277ð?ïÉØé2*—?x[É'ofZ?Zié²DŽ
?T:–ÿ^c?ty§$ã?u£yæQ(?ïŒëÄ<c?q¢ylF‡ö?x(ö"'‡?bb3^jt?€°"­Zº`?l./žï;?ï½`¥©"±?s³/™€3??j0?2y¸Þw/?Y
"€p?sY 6e›AGN3FGL J2358.6-1809@P¦ ºKÀR¹G"#ÐÀ:SãD8>À;Äꁺ?今ã¦á‰@.ÉA'?ý`ç÷K¿è£p™+pØ¿š¸þ{Õë-¿ÉÁ2\@:¿ââôxQ9GUNASNone?ïøAÝÅîa?M¾þÙý?1òw¤0£?3›Ô£¯:?EÿyÞc©e?FNòYh¡¾?ïGâlÇ(ž?"üԔ{Ô`?tÿ;{÷X?{)…ü	ô?'Ãã¤g™e?*š†Ÿ.?ï ®ûof?…RȚà'?"ìÝ>|@?s#-/]?'5¡±òÕ?€ÉƶqçZ?í÷ÜUY?¡²ËÏ?'L,-LjÅ?úš´y'?«ï3–J? sË*•'¿?ïðc§'¡J?™sCèŽÔ'?=Cí÷‡?wÕÐÔ³¿?Wçµ;¸š?"¾7#Pé²?ïÆ"þÔÿ?ucg©©?`ºß}<5?\n/ý?tÞ£Ŗ1?p•=Oï¿?ï—HȊŒ¥?q$‰Œ….?u¢oðj™!?[hRÆÄé?~¹+¶aXd?lcË1ÍÉ?ïR˜\qŠ?Ëe{PJ?`½SãÏï?ldÅhà­??‹Ê;8jsŸ?zÐ[¨jhdAGN3FGL J0002.6+6218@]SRÁmóù¿£äVAÀ8¸4t{ÒßÀ;¿"å­?ÿ®	&šI@ù8ö–Ÿ¿?÷;Q­Fʕ¿Áôˎ´8V¿àõø8Ðø¿çϟA›£,¿ïÿÐ%­õ­UNASNone?vP¦v¤ßŒ?x12Àç"?êCZŸ¿Æ?Ȁ¹þçÐ?Æ@Íhå-?Èlƒõ 0«?@Àçʪ·½?\5ž[Ú?ã¿°Ù{²?Å%^î;Ì#?Øx?dÍg°?Å'¥« ­4?WF ¾Ë?˜œÉ˜È‹?é¡÷ª­#u?±dz€‰.;?ÅÍ8'}sH?°a†å"K ?ÉÈÁ?ŒÂ
¨dÃ?ë,ÙS‡«I?¯XE"}?¿&ðž|ò?¬uø§1Œß?su=PæÊì?DI†]Þø?ëÀ~€—Å?ł­—°éË?Àb\"ʳ?ÅhÀÄçâ8?`íäy¼Ò?vqæÅÂÓ?å×[ÚNô
?¸&$N`X?Ô/l'g×]?¸IÞ¢5•?¨ ‡´Æß?šy9͍.U?逷üÂD?°?{ßj j?Ãôþ¼D%?­[ÌãE?®ÎQr"?'Ö»_ͬ?ëÐÜô/?¥ŸVñúí?¸*
Oñ!C?¡Þv9NPSR3FGL J0008.5+6853@]ÄOÊB®Ñ@Y»j¤¹ˆÀ9u(>«	À;e£Z»Ð?ýí,€çq@s[T9"?÷ðΑÈêÀ¿Äæ}ß+¿äY_쓀j¿î¾£Fõ¿ïÿbá*¼UNASNone?ƒízº®Ùœ?"Q'ó ïE?èX¾òæß??Ìó›-Bƒ]?Í^,Šfd¨?Ì¿.@Q¡*?t†'Ï"¯?•kѧ€v®?èҗϿñG?Å*:Ä?Ì$ŒHŎ?Äõ(m~Õë?¶֔`o?£L™©½[É?ç°#»¾T?±žéÂTb~?Æ4ÅU£å?­tŽ†æŏ?–ðÞeU¹(?¨gC¯L÷?ìÜ)Nám ?°êºnÊdÈ?³b}îUN4?­ôhó ¸?rºp
 ^,?'œ9¬~©?ë®Ì	!?É҇þ!ê?À®ü[Ÿ|Ì?É´–H	Ë?
?Š'Æ?˜ª¥Rö?é
:s™TÐ?½ÒWnY'†?ÉæÅ^ø?½YhgaR?À¬'ºØ-©?¨VÑ¡\l?æV84o?²AîY[ÞE?ÆÖe#œ?­ÏDélU?¬¨7Ù?‰É?—Huuß'?ì^lAœ­u?¥§
G&µ??­qõžã? <<Ϫ}PSR3FGL J0008.7+6558@]¦s>»ýr@¤á¼©iÀ9šCã…À;,rÉK8?ý—£FÉ@ÏzÒB@pp€p¨µ¿Ù»0(wÿ¿ëÈvaŽÃÛ¿ãôÄN4Q§¿é쌦t¦úUNASNone?·'P²u¿?³°¹û¼4?áC͍?Í=NÕ{+?טQ®QM?Ëò*g»-Ç?­ÓKäQp-?º}YЉxm?Ú²ŠÞ&"?ƆÖ°ë	?àɃ|KÕì?ÈD±Â§§F?Ølö̔]?²Ë؏yX?رø̖,c?´ÜS¥ßò?ÍÂìy:~?¯Ã1§ô¤x?Å5ùrXsE?³F@ ~ò?á eV#«´?Å£QOAH?Ò$8™yŽ6?½kɄ:Y?¸Ü²"³{p?¸×N·ÇLÈ?æý™D˦?É0±ItÏF?ǛB¾8ð?ÄUôs"Üô?ÃñýÀ¬ûC?Ç´¦ðð«?Üsá'Þlæ?ÄËÏú)–?ٓËy?ƇÜqŸC?Þ¨€ÿ¼/¾?³0Veæ"q?Ö*(Žƒ¼?²-X"š?ÆZ­çj™?¬ã¥5ÁôP?ÌBÇ¿‹Š|?±†EÙòÞ?åiÖ	Ÿ?·¼Z=•
3?¼2QЛþ?£ÎÉÙÖµ)MIXED3FGL J0039.3+6256@^c {5*"?º$ª.gF‹À9köÔ{À;AŠ[@	.êú	q@;epÈ¿Á'áÙ¬âª?ïý°3Rׂ?yѦ p&ô¿áä³Ä›®¿ïÿü]šK,UNASNone?̤N±ò_?Óº˜@Âך?æ™ð‡o©?Ôñù#u?²û3)²‡Ð?òqü5‰é?sÊè$ ە?£À˜sð5ß?âÇM"P?ÎÐ}·Ìñœ?Ú":9Y4q?Ν&iÔ¸‡?®š"æ¾?žJIˆÞÁ?èö"œ'?³AÝN‡ôí?ā3slU¶?²‹®6+,¡?¹0YnÜ+º?´­ß[¹œì?éÒAMI¬?Ã8"¼:-x?¾¡ˆßHa?¼¹Ÿ¯™qg?Ð×%€Ãÿ?ԃYðÐüÌ?äë}Oi¨C?ÖñšFg?µG'n?Æ*KL¸?"ù%a›?«'³_''Ã?äü¥ë6šF?Æ"Æ­ý?Õ^ëˆNÇ?ŽJ'??³À-ÈTs?£Ð&šXÈ?èacãn-?³Ò	Å\?Ě\©	ŠT?²Iøœ¯/?ÄïºQcä›?´ÎŒ'©?è.'`Ì/?»"a¿kBø?´°~Ò1ÕT?²=ì "lÒPSR3FGL J0212.1+5320@`ݧæšÔÀ•&Rz XÀ8ÊYž×ÇÀ;/`Ëò¥?ýyšóṙ@‡/Kòò¦?öۘð&n)?Lóp*¿Ùë»{–¤¿å¤þLf`¿í—*;:ØUNASNone?lþ¼Ì2¨?jz1N "Â? ææ?°ÃÜ(ÙiÉ?¤·r!Ïk_?°Œ´ƒÕ¸?‹ZMCù«²?¢™p£Ýéu?è…bŸ?ÃXð‰6íI?Î6çJ?œ…\J٘?žâ´­«¦5?Žé¹¤8õ?ê¶î²-lÓ?®—t™bš²?ÁGî¡]Þ-?¬V>îtµ?°Ë˜}"É?šÔµŸ?¾	?èì&ÿ½?²ƒK·K?Ãé›s¨2(?¯Ä'	À,²?^)ñ°yâr?kåRj´'?ïg8(¢?®•GÑ*™?›P€[¢?®èY"Ñm?žqÈ1lœ?£H{#IÌ¡?èTwÌk?¼ýi€Tצ?ÊßçËo™Z?»æ\.Ãѕ?­+îk9&@?žÆS¼½?êe€•ð?­Úª(Y¦À?ÀgncµÜñ?©›-ÒÓ?ÁAÁƒ?¡E‡u_¡?çý#p؉?«m'€ÌŽÑ?½"ayË%¶?¤V€t—rPSR3FGL J0223.6+6204@`¯âXOLn?ñצ_z¹ÛÀ7ò˜ëô°AÀ9àá"-nÎ@»Ð¸ê—¹@
ۚ?±Æ·?ùŽùÕÄm-¿ãÿī웿ہU§Éª{¿ç䌳w¸¿ïÿÖܽ}UNASNone?Dw~ÿ{³Ð?F÷DÕ,َ?⫃\Õ?ÎY.
è?ڞ½Z¹4?ÎY4ÄØ·'?S܄€ýÉH?u©À@"ö?çsÔEÏ(?À"çBòT?Ñ{^^ôÇ?À–~~'‰T?›•´"!O?'ïaà
e`?å«ï¯Ð½?¶°˜RŽn?ÒîДúÅÑ?¶tGÓèų?zi8ü<{W?xQzíl4ž?ähôš5Ä?ÂTeëõ»?ÖÄqèeé?›¬?'U‰É*6ì?1».Ä7?ãZ]Z4e?ъŽá|(½?ÙHZš³ÓŠ?ъà
F?kN}ø™°?zÖCSFå÷?èÉþ¾Xã?¶hñYiÁ?ÌjËÓá-?¶ÙJù<[?¥ÇS<ó8b?›RE®F5*?åžQöS5?³Ä]gâ?Ò
q«òjI?³¬Pºßc?vßÏ˒4ª?vÃxÊ#ø?æK« 4ñØ?¸†'bIÀ ?Ó
)€¤L?¸ö»ÌöózPSR3FGL J0225.8+6159@`¸åŸ+©Ò?ñîI9.õ·À8\'jPÀ:ç!éB?úÁ.ãÃ3@¿v×LØv?ü9´¡ÝµÓ?ﻼG¬š¿å"à…Cÿ½¿éäñ
¼¿ï|w@9'.UNASNone?R{\Å»O?QÅNnË?ÌmFŒMÎ?É
k«þ)?èÛ¢žâ?ÉŸæQ?aõÃ2'š?s‰*JQ=ý?à$›7JçQ?ýO÷d%?ߒÞ)?Ãѳٚª?«¬ìÇ8ð)?›
T:á¶?ÛC©÷Ïsµ?¹‹|ñ2?à£\7Û°ã?¹bâ½ßE?0µRÓN¬?‰m+CÓþë?Ý4ƒ/Iï?Œ8Dêì?àä8½ûg"?ÂÀä£Ðv?F¾ÿÇXi-?PŒ'åÀL­?Éð<Ս?È÷±¿wœ?é~Lƚë?ÈþÙlöÖê?"ÀÞ¢MJ?'^ßs}M?â'3VÍà?½cRF,q?ÚnûJäÇ?½ç•uƒ?¸?B'!¸?£\ømÔ?ÚMß±ÖÒ?´J4J*2¾?ßÙážÒ#à?´¿Ê·/ø?–÷IÚô?'²B†-L?Ü?´&sîK?·'»zé ?á+¶2'µ‹?¸¥`Oµš¸MIXED3FGL J0238.0+5237@a[&ÉÀ¯"á¬WâÀ9.ŸÇ±À;pÌ؋Fð?ø4eø­P[@ËÊÒ÷‰9?ý;3L³Œà¿âo5ãå¿àà¼;bµ5¿ä&â涿ïÿéò§}UNASNone?š‹­•}?¢;˜¥†jp?Üx»~¬êj?ÐhÒæ±M?àïDÔEg?Ёa	ìN.?r"«E•È?ˆÁO&jC?èÓ@'ý
÷?ÂÝ´üv‰?ÌÚ'aU?Áª¦öéÎ?̃m½?¼?®Œ4"H?âèüšè¨?´pY\Ò8Ó?Ç؟ö¢U¢?«˜"b­\5?µgTd:¥?¡IâôÖ?éP‰"DÉf?³…UpÉ?À
/«nâ?«ÇaiV¤µ?§Uןzy?°Îps?Ã?Ø¢ Ê-"À?·´²Ø7˜?â9' º›Ù?Ïñÿn,$î?‹Z™ÿp
?—*cúÒùÊ?éJ[ù·"?¾ŠÜ<e›?É&,åfK¹?¼-m1Â×?Ü_/"ŸS?±¯2> â?ÛQ7«?°ï"-ì?Á0þikÃ6?¤W÷]¦¬?Æpð§óO?¥©óÃ`Ü?çÞ©[X–D?®Á"vVÜ?´*‹G[=?^lgŸ[MIXED3FGL J0312.1-0921@gðwÙUqLÀJ.U⊤3À9ùíÓ­'žÀ;ͤ¦©M?ö2´ [)Ç@åYŒä)‹?ñ7ð<ªÒ?ÚDñ«±þ¿ßb{$¹rÓ¿â±ï¿¿ïÿö‰£q#UNASNone?Ö´ä`Ë£?Ò»¨÷tZ	?Þ8RBš?Ô"ºa‡§?Æ&4¥?Ê띁tx'?˺¨Œ?'¼?Ë‹²âQ*?á30¤7­@?γ–î¢B?Ïx"âáÈC?Á
Û?5û?Ò0žº¶?µxoì5Ò?àDúÔO«—?¸Q	ó¶Õñ?ʌo'ˆ¹?±–¾¯9?ÕQ´o«+	?¼è¡eB?ÜÕôZÒ«Ö?Á'*ôd/C?Ë°®m*¿?¼r*-¿Å—?ÜÐéßõ?՝䜢8?ÙãË¥õt?Õ·T}õ?˜<àŽ©.?Ë͋ƒ×:?Øöšõþä?Ð]#VœD?܌ÐÜ.*?Ïõà¥í?Äù([¤ýŒ?´üÙ_ß®?ܱF#?¶5úÿ¡F?Ù#j–fp?³ë!õ?ÄVø"ü¦Ú?¬øûX?K?áwï:_ø8?¶Qå7î'?ÖÖ¦»ý,ø?´q˜Œ'ð¿?¸åë<–ß?«ÛùGvƒŒMIXED3FGL J0318.1+0252@fN>ê šªÀEÑG®záÀ9ãpñãºÀ;îu"çZî?ûô`΢:@TÍ¿»í,?Ñc"šë¿Ï¡CS‰6l¿½F$ð'è¿åðÄ4,¿îz]ûͅUNASNone?¤ª‰J¬?¹L¹¥ªSc?êìµ_Y?Ê
E&¿v<?¾JSRžš?Æ/«÷j–?»ïÞ
«©?ČOßdÞ?äÐ/M˜w?Ïuˆêä?ÎþJÜzÈQ?Ī‰½Ø`?³´[ý+å6?¢~'?s@?èËJþDؼ?²	
¨ô¦<?Âø¦Vªu?¬àæ	^Îm?ϲid?Á€«Ìw"?ä""Úù=ø?ÅÃáѼ‡?¿‡ÓpÀv?»tXAŠŽå?£pz†@çË?¸Mcs'­?ê²²~å/¼?Í+üÏEÆ?ÀYb6Ü?É¥ŠÀI?З¤º'–#?ÎT®²IW§?âDͺ]‰?Ðÿ±[W>«?Æw£Sñ]•?º¯BSÄ?ÂD>¨˜v?­‰Zi$~1?çoˁFÎ?³tÂ1# ?¿øŒªY¬?©RÇÿܺC?ÚÙçÚfµ¹?¿}½ù<±?à¶ŒnÒ?¿=ÆL`?¯UXbqÙ?¬HÇ*\±PSR3FGL J0332.4+6110@a¤u£KÜ@'h	ԕÀ9¥¦&oÖRÀ;]Æ!·à¬?ö£câ"@Ñ•aüt@>í8}¿Ñ½±•¨¿ê?ùái"?¿ê"oGØÔ¿ïÿ3HE­ÎUNASNone?ÔÁ‡Ý?Éç››Ÿ?ÎK|(";?Æ(`úÊ??ÜÀe$5Ù?Ð|¤ç€'?¿ã½U?Á•&ž¶u.?ތA$k!ë?Ç¿;¬ƒ_?ÙzÏx'|´?ÈÒ.ØÒáÜ?ؑLVVh?²7àŸ-%?ٕ$è EŽ?²ÀÊÅg|?˳ôÈ?¬ø'+l?Æ

Ù*†Å?®­Ar/?ãï-—4\?¼Ä´‡Sn?˲8ržiH?µ"ä5}?á¡ë÷#?Ê9¢G+ýN?Ì'ÐöÊn›?ÃroòN?ÍP'•WPÛ?È-ÇÈoߦ?օ¦?Ì
'3bœÇ?×C0ΡZ¦?Ò^/ð¦?Ò7)Ï¥D?Ä-án¾é?á§Ö)J…?²³*ÝãÆE?ÔFè¶|?°QuÙï÷ª?Á="ÕíÝ¿?¤ÚRÛq?ÕÍã+>Ù?¯ˆGß(K?á1#`NÁ¦?±ì]¯à7K?¿?XðÜ÷g?¢™K§."ÍMIXED3FGL J0336.1+7500@`£~=Á@/¼˜¢"ÕÀ9TîDì™À;—éŠrµ?øÀaÖá@,Ó¯*.?øûiÁƒ¿ÓiՒZ9¿Ü0®.ã(•¿ä׆‰ÇiŒ¿ë)'Jê‡UNASNone?Œ!Í4p?¡öqSê²?îÆ?àh?¥'ýp"ò?"Xöà Tü?‰;ˆ¹™áŠ?Ÿ!‹d#uc?¯8ֆ ?ëFôE.)Ö?Àq:h9Wî?½ÿúûÎ÷?¼ê°W"¸?Å1¬œþf?²zٌ6?çÆ$×GFˆ?´­ê™ZgQ?·k€
¢&x?¡Iü"g±ª?·Ð›ãê®?¢`I^Rè?éðÂr"S´?°™—å;8?¸©Úқ"0?§/Mu͹?¶WèS£Ü?ºÓ¸ï·f?ìÜ2ÖtŸ?»êØóÃþê?†<ð¦d»é?…Q\Š»?·¬ì±QmÇ?·¹«hD"?é*Ò¢µÞ?ÁMƒ|²ê4?¿'¼¼š‹Ã?»aºø?Ü—TN?¶õ,ÆÀ?â?ß
|-*¹?¶d
h'Ò+?³ƒ³N´á?WANa´f?Ëwõ‡"•ù?§pŸÀÉ5?ç>'l 1?«$"?¸*=?®7#*ds?™îàNÝÿPSR3FGL J0340.4+5302@bXüø
Ã7¿ýí©¼&ŒÀ8ðà9'À;¸h'¹Ñ?üˆY«ìØ@»OÞ9±¨@ÚYO§ˆ¿åÀï7Ë¿îx¿ž)æ¿ïÿ}…^F¿á@ùðÏéëUNASNone?ÕïºvD;?ÏQà>æè?ÓHšŸ9Qì?ÍPœwÅ?ÖÈd¦PiØ?Ïu¨Xy=Ù?§'º8ƒPÃ?¾n¾­,üì?׋ÄÔÛ¹û?Êsl\'PÚ?âÁñò¬f?Ë°æ°VR%?ÝߎIƒ4?³s3§*'?бˆea%+?±O0œña?Ñné'UW ?²Ï¤9"?¹'NÓÎ?µÚ^ `Œ?ä\V²-(?Î×6å?ѧÇð¼?ÈÛèÚ°¡Y?ݟWp÷†?Ðc)¦Ó¥?ÌHb"«W?Dz‹Ë?Ô<²—†2Î?Íg
Žì?®­~IyI,?ÀZ
ã^?Յ¾"‡{?ǟ·0êiÒ?ãRI
Wi@?ɗº¸3sÜ?âsÔãià?²é"®‡Ã?ËÞúxùÞJ?°	>1ï?ÊQ±û‡—±?®WùŸÀYŠ?Î<€)í?¸¹°=߄k?ã
Ç8ˎ?'	ÿwã?Ōbø%s¶?¶Í$"í‰òMIXED3FGL J0345.3+3236@d
ʁ˜ñÔÀ1ZbwÄ\¼À9‡G.'º'À;†@@aïß?ùÄ9-D‰@øc^J8?þÑe*|*s¿¸'©öB¨¿éQDɼ*¿êÛåIxøm¿Üš¾ZԍUNASNone?êcg.?Á¡¡8R	–?ÀqS¿Å¨@?À'³\R*3?¨	ú
–à?§1$ÈÚó?ëä[1)Ñ?Çd6ðEç…?ªp£&\f?·2
Àj—7?³¤Ôâb8Ä?¿·Žœe?⵩õSËü?·c|?˜P¬?Ï{"ÿѱä?³­2i
ÿ?Å­Ä*ß+?±šð,÷z?â¥ùK'h?·bÞ­±?ǶD¯ XT?ÃÚÃ|äO?ͱÖ$B??½¨k)ÕÎ?ë¶yK›^ì?¿¬"â¿l+?¼xÉ;.™?½ñáëS1?—M±ŸÛä(?˜e«óß?îvÜE:ǧ?¶"Ãi??'ÎŽ»;¢:?¡Š"a·|š?žUè ÛÞ?®;t¯±1\?潸æD?µÊëWC·?ÇêºÜ½ä/?®ËÿÝÆDH?¿i"X½"?¬ÌÕÊçQ?éaPì›c?µr7Á?Á1¢ã"e?³9Åíÿ?±1¯±{;?¡aõ€"¦—AGN3FGL J0359.5+5413@bˆLYtæ\?ëæðY|sÀ8nÌ¡-â'À:÷c°©€—?ý3ù;듌@Ÿô§‡C?ük—›<±â¿Öa78·"¿âi‰Ë45+¿æ7ÛÓ>Æ¿ïÿç—åu¡UNASNone?dS¯"ąh?rC¼×…B?ãQЪ|ë¹?Бΰ7üØ?Ù3·L²á?Б<UM'?4ݶwî•Â?V4° l'¹?è`ÕT©þ?À®u18î?Îr;Ô?À¨j#חù?«©/¥êGÍ?˜5HÏ6:x?èz¿ñ"yÂ?°¾ö\ì~¿?Ç*´Q´[D?­àJp *k?"Ôa'>Í?yý!b(#Ã?ì(Kž9˜?«4JNF£Â?¼#Ûc¾k?©Ê¦fbˆ×?U>†) Ÿ?c­á‰L6f?ä	Œlp§Ä?Ѕ"µÀQû?×ר )z?Ѕšth?U12«
ž¬?h›¯¶z?éj°Èg/?±·öiÎ?Ê*Ý_}OG?±©"NsLö?À/7÷¤M
?§Qaì`S?çQs1S?°ÚàZb?ǂ;•=¦?¨F‰:÷"?—'xEà)¹?'¡w¿kC¨?ëãßÆØÃ?¤9îWžé?»#·Yú?¢H­Í;MPSR3FGL J0426.7+5437@bÛ¾ ºK@ý¸ýâïNÀ8'£A¹ôÀ:¤UÖÌ*@PŠÇn¾ú@•†ø,L?ýæðõvO¿ÌÖùͶ¿ãUº¿ìÝõ›W_¿ïÿDUNASNone?"&®Ú7?™¶ñõúcK?ío­1¦ì?»Iˆ0æI?°Ó'
àØ?¸®œagQˆ?y¶ÔÐÂÉÀ?‡KªMp÷?äÔt´1öG?şï£UH÷?Õð;D'Cš?Å´RœHå;?§f"Q/ˆß?—›&e4Ê?çEÅc?¶"ßô¨Ñ?ÍØÅö¼?¶
'BFÓL?™.XKÿ.Š?ŽšgR}.?éSrë|\¿?¶˜È@#›6?njiI3"q?´Ø+/??Ì££¬¼?—y`4yE?îÖò·å?³ÿ¶Da?§›	͇}z?±U"e³?Ð×FÃöÊ?—1µu;m?æϵBþ"€?¿-hC
k¿?ÑSˆ{´?¿Í&+ë?´šÎU(Ÿˆ?¡ú<aN1c?縩w2;'?²:úÑ衇?ÆÏòøkÈ6?°pS»Ó{?¤Åf#÷á?'Sìíý¿¡?ê
qKOgO?ªrr™?¤áI97?¦Kï$PSR3FGL J0431.7+3503@d·BZîc À!Ûà›¶ªLÀ9Aû§««À;"n@O{?ö>?Þ½:3@cŸa¯@¿ó£%^‰¿æcb	¬Éo¿éIjX×v¿ãH VÑaÌ¿ïÿÃλ(NUNASNone?àT'c`?Ê%êØj?ÉÖ̊² ý?‡зp¢³?ÓñlòÐ?ÇÝãâ»!?ÁÅaž€‰'?À^°qnώ?ßùøϊo?ÄÏfW‰?×#VbH…¼?ÃæYp‰ªä?ÞÖ*Ò'C?³žs[tùZ?ԉ¦Ò'3Ÿ?±µ{©Aù?É@]!]¹?ª,éU	@?Îò¬&uF?²Ch'>=?ڕ˜=N5?¿%zÎR]ñ?Õñ`lž±(?¶f~nç‹?æÀ#aŒ•ƒ?ÆxØäˆ*[?Äê@8M?À¾{Ë?À[9•*¨?ºa
œf'§?Òu7´,7?Ç£/ɶÐ?Ûò«ÇÕ¨?Â,ðXõ?ј 'þ!?Àh_Þh^?æ85cd(t?°•NÐÖC?Ê+¯[L×Ê?«Ë̬|?¹æö.EÏ? 
^Fä?×%*U'Ø&?¯Áû'G$~?Ý¿ÒPÖ?²:-\sb<?Æ7}/U®?£ïQ>ðMIXED3FGL J0514.6-4406@o/-w1ÅÀA²DêÀ:å	ÚtUÀ;Õâ˜,ž?öýOòÁ`@K&Ðú.@œ¹a`B¿Øda~u%ò¿æñye­¿ý¿ïÿäÙ«Nð?ïÅ7ƒ5:[UNASNone?î…jU3c/?ªuý²B¾ß?˜¿¸?¶Ÿ?¢Ý"Ûëzl?–'ý ¼3?t&âO½n?ïqüF."ð?šv-îJ¬ê?nŒp$£øì?ƒs95fK\?‹ÝÒböµÎ?'荅‰?éUxEÈu?¯÷Њá3Ñ?ÀÖÙH¹¶?©@ÒÇÒUè?µ™óï?¡£¨l>nZ?ïDñnH?¤'ϖšz"?tpuŸC›™?•"©Nøž}?—Dl%? ÀFæö?ï*S¾ÌŒ"?¡Ž|©¨Ð?'&Ww
N?šÈS £êz?ƒù¢fDt?‹,‰wÿ?ïÏ
IÈ(¬?†^*0>Üì?[Šï~ÈÈß?v=˜
뷇?q–ŸOwGÆ?x££'÷°?ìp2Ü1æ?¤»ˆŠ[@Ì?²zvIЇ? m9]Q'Y?¤ÕÝR.?•igÁ"j?ïå¥>qˆ?SïÇ×­?QßT§‹?xJªðšaŠ?aÌ8£m¬y?t×pá\Û\AGN3FGL J0537.0+0957@hiŠ	ÞÀ'(÷À9˜K»ÀÀ;2(@éÈ?÷¸ß9áÎ@ÒåE°a@M:*ž9<¿àNéÐÒk¿ên¹ª¿ì\kñô,@¿ïï–û¦÷HUNASNone?ï²ËÆßÅD?÷ï`+¬?l@áBäÏÎ?z"9SôJ?xy«éہî?ˆ¹ZáZë?ím+"SÎ?·¦B!;#?—{}j]½?¡ÐÈ§5í?­o"$ö?²/¥R«
À?ì™íAêä˜?£Ýg®Úí?¯y{£Üµð?œFx§ŠÏ?¦ç°:d?–ñxäµz?ëÃI¿—Ÿ?¯¼è—ó@?ªÒªK1p?£ã´n&ç/?´|^ێ£Ë?©Ó;¯a5?ï¼-ˆœ?"dsGDÞ?rŠïŸm²?‡M‰óË?n½ Z+?"e¢µŽÐ?îå*Nˆ#P?¡6ópËP=?†&à4JÄÑ?†j…Çå
_?˜GFŽ£?™‰LR: À?íÙ­+$y?™Â	sró¥?¥Ö%ÈÞÍù?"NÁ´3Üx?™'j?Œ:-ˆÞ½?î`…ZŒ,b?•…!ûBúþ?žóc-"š?Œ²Ï§pèc?"ûñ‡ÕŽ?ŒÏ>K}"AGN3FGL J0539.2-0536@j5®h]·kÀ2›bÇut÷À9@[9âyÝÀ;3whí)d?úAN*…@WMç'@oñ§ÍŽê¿ÄеuÔS»¿ìÝÔ'¿çžr'—ír¿ì'äuNÐaUNASNone?¨[{ˆ®Ý?©ïkþÃÏ?èê"PnU?ÇáAŠ9g?Æ>ÓÛú¥?ŏ	Kiq?¨¡f¯›ëW?²Æ}1Sì?è¡å9ïÕ?ÂÖ7é•O?ÇSjÀéÕ?¿uü'û"?ÓèòÐË¿?°ðmý
Ñ2?ÞÖÎ@ÈМ?³¿wÔÁÇ?ʀ}ÜØ;I?­ÊxTgšË?¨kIê½4?™í½í'¾T?æp¤ý?À7fÔJo?к]ú14?¼‰#ªª
/?ªF)®Dä?°Õª¥õ6?é÷i˜ljY?Ä_dK{uå?Áañ&?Àì6C!ׅ?Á5䦜ü?À³ï¾
ßy?æ6cã:ˆ£?ā¨r`«Î?Åð‹°o@w?º`ÈWG?Û`aäx]?²yÕÇÜÈÏ?ÚoÌëoi?±³'u*Qø?Ä_¢a=6?¨€ðŽŸ?·.V²¶? Ý©`X}?çõ=%>AÉ?²~­Јk?ēài"?ªŠß=MIXED3FGL J0541.1+3553@e²PÅë1<@¼÷S½À8¹ÈÓC"À:É(çÖz?üӮɺe@{%Y*éŽ?þáñ¿Ò̒…(Ht¿äh³Î¶W¿é¦Îb›x
¿ïÿÃÖȽãUNASNone?ûWoj«v?­,E¾?ánýÐOä?У›éž?Ü4Iœ?Ð¥jxë^?`šOév¢†?+' ÌÅÀ?蚬i³€~?Àšô2cÍ?ÍRå
±Þ?ÀŸK›p?±dShÕ"ÿ?ÉӉ"—?æÔ ²?µKÿüD̝?ÏMqÿ2
û?³x
m`8v?Šï!†C˜µ?¤³õ¯?ê9³D:˜?±Ô•—L$€?Ål—®õ?±,vfÊË|?'Îx'úo?šžؓèE?݆ûd?Ð&Âim?à®6c`Å?ÐJ¼A9[@?zeLÒÂi?'nKë™t8?é¯ç±!?·Ö%ÆKü?ÊÞBFï?¸	†NZ£?Æ9ÑAŒ?­.¢o>?㩲Œ7cø?³ŽäÀ=Û?ËdŽ
ä?­e )â?š2y‹?†›Jnš.Ã?ê?¦V‹X?§Ò' ?ÿ!Z¡??¦d".nÈùMIXED3FGL J0545.6+6019@câXOLn@/©Á/	ÙÀ9'jËΠÀ;®.Me?øKÂ@¨^ùŠšù?ïdã&€rV?ۇŒ»ÿd¿ÓÂÊ$ú¿ÙWÍW\¿éƒ'ÆSÈUNASNone?ÔÛQBpp‰?Êà'‡+­Ù?âõòt*[?ÎWåÇ ?´ã*ôT¹?³ig­ÑC†?®¹9þ)?³f\3}H?é,}SŠ8?ÃD;G˜‰¾?ß¼Náu·?À™áÀ(W?Ør–üÂo?¾ý´ÁŠ?àAy\?½á¿B9z?½ýj.0ó?¦'æZ±È?ÎIP®¿³?¶"ÖèvÏÕ?ãˆÃv»"?¾½Œh#?Ó£R;?³¦}¨ñR?Þ¡ å¤pH?˵ÃaÙ?ÛñÈå=?̊0Ê<š?¸ùµKwè?¶m˜Žö‹4?Ä˧è?¿¦5Wø\?æJÀuë?Äm*¾''?Â	ù"wÔ?¼UŸH?á/~ÅôZ?·R5NM?×îûÃ&Ó ?¶k'÷¬úh?¶È U5®?£ÔE,"?Ø[ˆâg=Ò?²¸‹õõ˜§?á­Kšˆ,?³LWõÉëþ?±(êj®W? Æû1ÒšMIXED3FGL J0634.1+0424@iáXâe¿ýRøBÀ7Ȗ'•¿À:'zÁg>@Î郑Åe@¿Ê˜@"—hk¿ÓÎÿ‰"ðâ¿è"Dtñf¿ë0yTª§3¿ël›ÿÐZKUNASNone?'
°z+I@?'>k,<w?àûøŊJ?Ñ «¿"ˆ–?ß=šŠ…T"?ќ[Hƒ°?9&Dw>™h?ZZœéc;#?çʎÒsÞR?½—}þ'¨?Ðd˜É˜˜p?½•	£(é?µo¼ c??£˜‡-¹?à¯î^†¸?¹	æèê«(?ڒ±ó)?º	•ª÷ï?¥"p6®œ?yméÞ?êvuÔ²?³°ã[ÉCD?Å
M¿ë+Ì?²àü\®íï?€‹^Ç!ne?†g^äu?âàØEâôh?Ñ}D¹ÃZ³?Ù¹ô}•×î?Ñq«A?n?EÒ¨I`ª?b,™Fӛ?çê-hC
l?¶0äºÚP?Ð »ÛҒù?¶90ä~Ž3?²wIk6?«8'tž6?á€ñºÔ
?´ŒVØ7?Ó¦šwÔ¼Ÿ?´`%öü?Š"δ×?zʐC?ëÔV˜àX'?¤Ò5ù€6?¾±`­^?£!.NÍšPSR3FGL J0637.5+0418@ið9–ú'è¿ñßX{ÆJÀ8ÅÞSÝͦÀ:¼hA1ùw?ú¶dÙ"@@p"Í@zlnh¿Âۃ«¾οêCnJœ—Œ¿èÌ׫ðV¿ëÚõªµ/UNASNone?×Imœ»	?ÉVaס4?І?öڒ?Êc>¤ç'°?Ø0S^:·¦?Ë´´ûÓS,?ŸÑÖÐEx?©ÃîZO҇?˂˜"š?½ՈÌ܁?è ËA‡^Ù?Á¥Ï?Öz~xxY%?µ©/]Â|2?Òó'àÆ1†?²/ˆ.x"?֑ï¦ÁuV?·9W¡S?Ñ×|Fã?¶ëd7*?Ðûšêk]
?»G‰"öF?Ý,é` ?ºè™W»Žó?áÅ]?Îðå6aL1?ÏWč
D6?Ɉd»Éø»?ɐƒP,X?ij1‡ÙË?°À"=§?»«""ˆHõ?Ði€ÿ'< ?¸âvøYî^?å³.ý³8k?ê_1
[p?áo;‡É;?¶CÆ9/?ΐ5àÀ'V?¯<H}ÉX?˲܃¿?°ùȅú²7?Øô˜ÍZ«?³Þí'%m3?×Mu\V ?´imUÄ?нHþÕ?­‡«r™oMIXED3FGL J0641.1+1004@iY;%oü@õ¡lèÀ8·àªÐ"ÃÀ:¾­'tâ*?øz0gQ@†IŸ0\i@ªñó—¿âE":{•¼¿çOx1P@E¿ï¹8Î?Ð W3¯tUNASNone?ßÞ þcƒï?Ó2<ø˂?δ®·§»_?ʙÅP#%k?ÐLJ¥Èža?Ìã•Åq?àYi³º?×Ø×@²çb?®ƒÍՈ?´$¥6;îq?Ü\´Y?Ö-CkK?ÞÆ`ñ—‡?µÚ‹Þ7[Ë?Çrf¿þ?«vW"ú>?Հlüˆ¶?´ì¿g
Ê&?à\Cv¼
Ò?É؆¶#N?¸jüü¯?Ã×ʹw0?Ù,º?o?É!–—uk×?ä@¹?–?Ñ
Å^wZ?ÄÀö4¥#;?ÄwºŒ-uY?Ê>Šæ^ªl?ÉGpĎ:?纬˜h°Ý?ÔSÝZÂ!?¢–{'ÿn?ªZ@LÓ²?ÌoɾœÕ±?Ò&JEã'ò?æ³~1n–?°'¸±«Áâ?¿²íÉ?¤E˒^?ű¬³°NÅ?©`âyÝé?èyŽÚ¬g?¼¡Ø±¡<?®ñ‰ÇHç@?³«uå	…?Æ]b#êž?¸á{›*AGN3FGL J0704.1-1043@kýHýŸÓoÀ¯"¼
êÀ8ƲœŸÞWÀ:W™?÷Omü]@
µEw•Ü@@-Ëë%¿á¨|&Ö¿èû0•ý‹d¿æì.wпëAßQsUNASNone?§:*ä©9)?£{Áە?Í
³ýsß?ŋÁA?çHðRt'U?ƸUf¹Èc?"Äó9žf?¤X7[Š<?ÜÍn³<?Ä»cŒP?á]ñ®"¹œ?Å¿üEÊm?Òï"Ö?²…ƺOÌ?ÓÎî j¿Î?²ÀWêñ¨?ÚúÏ¥«\?µËx¦ê@ú?ºj´ÿ¦"Ó?¥èðÚŌ?Úsî/¯+b?¼9gïlMË?Þñdg/©?º8CZ?¹ö–Õ4r?´CØGÚS+?ÐÖd/÷·?ĬP3³¿?äV+Cí7?ÇUfïxHf?«´¤8¹Añ?¶áZ»îï?Û~À¶z6?À$†¥©¥ß?àÁö\4«¦?ÂÆY¶T»C?âºË7?²¿¬»¥×?Êpÿؤ¹?ª™҇ˆ?ʦ¬ûSÑl?¬W䪀?Å[÷0½Pó?©p±sùù‹?ßÀ9¾4%?±È>2[?Ցʩm2o?°(NÛ]ÈÙMIXED3FGL J0711.1-1037@làuöý"¿à"5Iè‹À8õLÓi©À:˼zo1ç?ø—h\4ß0@
?Qkr•@¼1ÊèF¿â{ý3¿åÀ´¼Œ¿ì?_®]ÃL¿ïÿh¶«UâUNASNone?ƒB}JðÊ?"ØŒ:äÂ?Ö°"UÕJ?Ì>j(½¹_?äZ¬-`?ÌI3O¸¤ø?RnëG©?j0QŽ‹q)?á"wüï\ø?Á55]/?ÜϗTgX?Á?1}?_«?Æ2aÇENi?ªmU¨Yú?Ý»I}ގQ?¶@ÖʳŠ?×+…ž~Êz?¶ôðú çä?¢×M'$Ía?"ÐÎ¥o.Å?æþñþh-ï?¸9ð¥dÁ?ÏNd¡4,?¶|Ú¦GD?šz*¹H'å?›Ö¤«ö‡?Ô:}"Ö;`?ɵÁû/C?åïß¡eÁ?Éð·®â?q`Ð
µñ?…Ý2…O¹?á\v­¨¼š?½DsÚ9¿6?ݏcØ?½ýÓ{£Ëˆ?؄ì–õ-?±¬2ïÞ£#?ÖµZžö¿~?°yoµÀM?ПÊf?®ÒªèÂ?²'Ììocí?›¶êï>ë?æ¯r†&"?­åIûë?ËøÏrwx?ª=ØyÂþMIXED3FGL J0737.2-3233@nÚðEwÙUÀ",Ë:%–À9iÃ9À;6~=ó€–?üÆ~a"Õ<@¶ë+g?üòok²Ù¿ÖQ'[0õŽ¿ä½óñ‡¿ê½?á{¿ïÿÆM¸UNASNone?¬2ÚÀ!æ?ªÜ<e›:?éwMõg‡?ğ
Â
|?Ãƍ:*?‹BL×?€]P¬*–Þ?\íåÍÙû?æ̦e>½?Á|õ®Qí?ÑãÈ°øÏ?Á4Ÿ¤ ˆÌ?½}ZÉ¥%?¨ë"Ⱦy?ç˜'쮤?²é53­™?Âà²æO]i?¨p²a%?±`¿uó¸y?™$ö,ã%
?éÿþ
ȧ?±Ï$vg?àL*ê?­ÀïÊa?Ã×i'ik?Ábh'8ø?ç	ÖD½Â?Æ]ÃYÄ?À=h||d?¹ÂŒºw?—Õ4vësö?šºK"?ç/ym‡Ëo?¼˜òTƬ?Ð#¹ÝJ¸$?ºô˜	²Â?ÐçªôŠÖÞ?³^£k€?ãI[0RX=?´N´Ãì~n?Á=U ñR?¥W"e·?ÂWÈòUP? KÆǸ†?è$²"÷÷?¨Sc3¾äÑ?º/à‹y#
? å4àxPSR3FGL J0744.1-2523@n*Ûa»û¿æ\°ožôLÀ8u~ÚÑrNÀ;
üaåÎ&?ý
ƒqd]@w@Úæ•÷?ÿ ÛÍp¶¡¿Ú&枰¿å¾3Cû¶¿åþs0Z¿ï‹žw"¤UNASNone?¦FÜ
Ù?¨¼Ö	·cÚ?é-shâË?ǘ9@Ø&6?Ÿ|ÚW`?Å‹'L0k?^ÌÅË誆?v³Lwï§ ?á+J5Üu?¿»(Þ#??݊ž4?¿Áã»ß?ÑxBMú¬&?³W)ÈÖg?àå#C.±w?¶ýqÐêÎ?ÉzîWOáÙ?¯Lê) '?·
í-þ0–?îF3ý)?æ§ITªÃ?²û°ñ47?ÉÝd!vë?¯³×-Z?²áhî
r?·íý	…®¹?éÁ-@;?Å:U¼J°?¿ß:5?¾S¦Êsoþ?}…–WÝx?'žm}?ãð©ö³ü?·Àrrú?ÙxR'|¢?¶É<T²r?؃Ä;"ç¿?´?
|Q?ݱ•ÑZrŠ?´ðqVÂJ?ÕKæ!Kn?¨±ÒýŠ?ŘL)EÀ÷?¡··Å~¥?ænU*©ÌÃ?ªçÍêe+V?À®_,ÿ? öTΗòPSR3FGL J0758.6-1451@m>·€4mÆ@?W´ûßÀ9¤¤ü¤*íÀ;"¥]òú?÷3*#êì@
;T˜Þˆ·?÷©æU´èU¿ÑËÁÀÔǿ҄‹rù6¿éªí_Gò¿é¿jœw^UNASNone?¼(g/íŒ?¶âÈ¿T?ä裛-Ëô?Ì3dÓ¶˜O?Î\Ý_°Ùk?ȱÁä;~[?À6aäªÈ?Ã?iëD÷?â,·|Fä?ʛ‰ Ô%?Ӌ`"fÕ?Ç»»«DðS?Öýl¸÷.?»Cz`׆?ÝÝjî$?»ùF[Çè?ÆJúO;ý\?®¨³‡ö<?Ä@îXsð¤?°l¬î@?çOšÿÔ?¹È'ã>u©?½KQ ?¯â?'Ì}?Îÿ0Đ`?ĉÍ1)K[?âåí°=?Ì6…kAõ÷?Ɉizþ¬?Åèt•u"ú?×õ%²}Qv?Ñ$р»§6?Ú2ÑÛ̼?Ë°	Rd%ï?Ì
N÷MÜ?Â/˜O}ÒÐ?⪙>³wš?µ¡"îg?Ó<!TŸ¦?²±3ØäL	?¼®E…ě?¥+4»b[?×L5R0Ó?± ô4x`B?â³î73?±ñIIº"?².MϨœ?ža€žy"MIXED3FGL J0839.6-4133@pRJB®Ñ9?Ô"}Œ.À8†à"&þÀ:šˆŽ¯ZÌ?ýU9Ý@ÜzÛéJ\@™V¸É_°¿hZÀ
¿íø[ª£é¿ëYb…U?¿ïþ/¨0­"UNASNone?‡­åîì8K?"dÎöBž?äÇnT­'†?ÒO-¾î×}?Õ³´'drñ?ÒCæ*',%?Nu"ÞíV•?gPwn¥ë?໨àçêh?Á¤Ó´¦?Þyssë	N?Á±$À~¶?ºgš¿š›]?¦VCîí3?ژw'€4?¸\
¦ªÑ?ÞÍ¡¾¬"³?»'ºR!?˜þX¡[ù´?‹YB6gb?åZÇïã?¼ÑG«²²?ÔGdåÕ(Þ?»Å~öf_l?~î2ÀJ)?Œ—°ÝG;?çÚá&dÝi?ÐuYYž¾?ϝ	Ñ&¹?ÏøˆÒÌì?hg?ŠEœú?Æèš#Pi?â=²Œ|·?ºÛ¼Ô²v?ÛSÍoèxØ?»aéÙ;ßÄ?Èùà+Nbd?®g
‹pña?ÜWRŠ]ß?µŸý+9i®?×+ý–»1?·€רfõ?¥úüó̏?"·´<Z?æ{ù§¥È?°êtC7§?ÐH­;?®ó?Œ¹µMIXED3FGL J0847.4-4327@pxdZ¬¿—»»`|;À8DmØJ¯À:f]@L÷*?þ(˜¨-G@îþ—@ã?þÁyŽ°\¿´Nµ—<wI¿èg×Û|E©¿ï9EÍÙV?ÁY­Ñ	‰UNASNone?ÒÔъîþG?Ò½S'oZ¬?Õw…ÛÕ0ý?Ñ~'²!?׳¨šN±z?Ñ<@ÿ_Ø>?´[ìçì°9?¿Zf­!ûl?¶b©m	3T?·~ËN¿Î?ê¨-5˜=N?ÄxˆÉ'±?Åýüü"9?±
Q²†AÑ?ÏK'{o'?³å]¬øSá?â­Ò![«‰?¸ëB'?ÑS¶E;?ƁþGn(¨?Àwi÷"J?Ç,¡¾×Ñ?ã_ï¦üP?˒1Kã"v?ÉŠZó|Ë?ʖÑbÛ?߀ý–n@û?Ñ­vǺ?Óð=<Ÿ?Κ"¼N·?ÈïSššd?Î{¨À±"?¹D%i÷˜?´hùóßP×?曦Œq=?ÏlԐTe?Ó0bW|Ø]?·q'zqc?ЪP9íü?²X|K¤ã?ܺóXI9§?¶ìˆB'ò?۔ŽyÍBá?ó,2
l?¹sQŽñ~?Á1ëҐJ?Û·ÝkD`?Å2œ¬æMIXED3FGL J0851.4-4244@pvü;Oag?ïÇõݒAáÀ8UÛ¢R¥¿À:iΐò++?õ¿§@f"@
ð¦z'¹W@€'µ¦•¿àÉIY²›@¿ê¶år
3‹¿êØ[#*¿ã{Ìй҅UNASNone?žº"ó/½&?¢×¹€bé?Àô'¾¤¯¼?ÁãvvBÁ5?êÍ!è¡ÙH?Ölº#¸þ?¿QÛXłÅ?ÊlŒÎ¸"?ÇlU"u:?ÂsÙî•ÁÀ?æ:¯O²Y?Ì?ù#[¾†?È&ӓæQX?²â'ÿ'¿?É'̏\¡8?°öÊeû0?ã¬W÷¸³»?¹+Ü5HÑ?¾>ýÊNJï?¯¦·àèžÌ?̒S\Ñð¬?ÀÚ	"[õ¨?å‹oºw?À{ë«+´±?º/æ{ä@Ì?½\ÿñxŽî?Æ<€lÞ?ÂFPbTD6?ç*ßÐh@d?ÈO¢¬×B?Ð$Ó-'ð#?ÒÎÍEÌ©?ÇPf›{­1?Á`¢þ®W}?â|¢?В¬é#?Û#©¸u§Í?·¨ &-i¯?ē\©#Oe?ª®®¨´?ڒ§òø°€?·šµàb…û?ÈчÍû\=?±Á+,IL4?Ò]'±ŒÄ8?·u1PŠ%?àœÔ³ºÆÕ?¹Æ~ÿåSMIXED3FGL J0854.8-4503@p™¤ü¤*í¿—tR§¬¬À856£*<À:ŠX;*xz?ýã!°SðB@qíVD?ù-Ö|ùÑ?Ó¬¨Üì!¿Ûɽ£º¿æ4È«ø8¿êc?Dä`'UNASNone?t¾1^à˳?sPêÂ?åüJ¢KÕþ?Ëð7Ô
a`?Ó´qõn_7?Ëî¤M|µˆ?DÌù{'¸`?`·PÒ$U?ß¡~3¦dr?Ãg"t°<Z?à*
¨	Hÿ?Ãvóq§7<?¬.©¥o)?Ÿôq¢ت?ã g:»'?º[`–÷0?Ö:
üÜ£É?¸Zæ¡ýCÍ?œÖUó¸°?‹ü֝£?åJGZ÷6G?²iA8Îé?ӞêÖq?²"žšÈ3?zKkÃ?…˜ÁN]i?èý¯3ì?Ê l&nԟ?Ë98_0ÖÑ?Éé|:¹?a:U-hw?v$[]­‡ô?â]‹¬&w?¼b€_®2Ð?Û"süë½B?¼Ù#'1§?ã''Á'?­¥¾34"c?â[\rÑ?µibÀö¼?Ò	€³TçÊ?³ˆ 6W‡?§hŒ"©?'†éRd\é?åà–ÜX?©Ê,'#¦?ÑN^ÄþĎ?©)bÿóyMIXED3FGL J0855.4-4818@pÂq!«KsÀcҢϣAÀ8gQÌ{n5À:vh@Žf?ÿ‡	½=ä@,/±™Ä@7ÒT¿×H1Ð¥¿êtþÙ»7¿è0 ûHòH¿í¨šêbÆUNASNone?€Ü˜ŒFQu?½°;§ä÷?â÷pŸ?Ðhj#חù?يZªÖ?ÐR!K]l?Iφ6?cjdÛs?ç.¼ZR ¦?¿Ë(÷‰Ó˜?ѕŸˆŠÂU?¿ÇFÕ@Rš?¹»Ì°ƒ|2?¤Œ½Õ
'?Þœ;#[i?¶8äíá?یp˜»Å‹?¶«ý~@XÓ?ˆ¼tØ Å?€·x1~úõ?åCUܚ9?¾~]-`>?Ô³p &%¯?½õÀr1±å?b%"ŽÀÁ1?eG§Ëâ?éô3"ü]?Æ+ÇÍHÛ?ÇæQù¶ª?ÆPO<—û?^5r +‹?rµRÍÏK˜?æâkúïá?¹Š/ò –Å?Òò™åï´?¹œ³sÔ?Æ/Ñ<PÆË?¬†uØ}K?àÂ(ÑQä?³Íξ¢9<?Ô¼"4øÓ?´tòùºÊ?ÒÀa‹×?'E—…3ƒU?èŽ«v]L?±Ú¡AÞ»š?ÍЙLºR?±ŠŠïPSR3FGL J0857.6-4258@p…"ÿCAž?ûP¨È%žÀ8yÊU#HÀ:~ϟåãõ?ø"Íû U@k€´›R¬@ä€ðÖAk?¡
Â0h¿æwúٚn¿ëJ¹4-¿ì'ïHͤ8UNASNone?Æp•Ð?À䦟ÞÏ{?ÜÍì(ÿõæ?ËuÜMüÀ¹?×ú?Ë!‰iÃ	¢?ºÁpùy?Ä†~½Rå?Ò-1o>?‹û¶Å#‹?ã©d9)[2?ÉxҀ&<;?ÅÔ&w&í?¬¸Ì'Ø•‹?Õ2Ï=Èëõ?³pŠÄI?à ãX0©?µýœÞ©‹X?½WæÆÈü´?§Ù¿Qù—½?Øöß¡Kû½?»?jl8#?ß³&­Å?º0t–C½‰?ÏéþpÖ#?Çj÷BRq?ß´ÆH¬Ë?É|W|Ç.†?ÐW]:~è$?źb€#ž?ε¬8œmx?Ðþ>.ŽÞ«?Ó/zcjÖ?Â<5ª½?ݕúh;}°?Ëï]«µ?Ø ½¨"?³²|ò|2?ÓEÅõ?°6w©¨?ԚU|ðQÈ?³æéPy?È IVê?­¼
?ÚçÝ*?²!šn\¨?Ù
ïô¼wb?¯ü^ƒðšDMIXED3FGL J0858.6-4357@p";dZ¬?óN~é+0À8;IàâÀ:o²'ž«Q@Ïh5ã@(ب"H?ý$…(0K¿ÐZ"¿æÆĤNT¿îˆ
Aпà.Ý
6ÊBUNASNone?Äø%Uˆ?Ë·3m72?ʊJ,…*]?Ê)ý 2?äd2ÉDÇ?ÑÂ`¯?ÈÚç;QÔx?ў/[ôX¾?ÇDm´¼??Ãê"ۚ?ãø*Ä#ÛÒ?Жa·L?ÌÕ<·/E'?´±‹"¿dÞ?ÍCÀr,?±€ðö	͂?áyÀ±ò'?¸_Ñå7@?º-?ÂýZ?±ýQ¢O™È?×ýiÅ
?Ì98RNMã?á3[£%Ñ?É4{$ìü÷?Ç_½»óò½?njÀJæáª?×ËE@Ún?ÍΧfû{{?Ý2UÜÅ,3?ÏßòC~ÚÑ?ØôˆúI?Ø!èe¸?Æ©çòvw?Ŧîꌃå?Û¶ƒö«S¼?ÒçÐú×?ÖÙAF¾£?º_î–åÎë?ώê-¨&?²u(J´Êœ?Ú×É¢mJ?·Õ4bMÌ?•º<§?±Æýçu:W?ޑv«¿F?Ã1;Tr{¦?Ø#þKcÅf?¿Þ¢Y©MIXED3FGL J0901.6-4700@p½o?Rü&¿Ù@ÝÀ»À8 Eð¥À:OY•?úónçê4'@	Wze¤?ýckw¶¿ä3ˆ"¸$ä¿âš¨Éüý†¿èá›Õ¿ïÿ²§ "ŸUNASNone?€X'æ£Å?‰8è5O=?äQAEg	Ç?Ï4XP'ÙP?ÖÚ¸Þ-rT?Ï(AÓ	&ð?sÃögågY?‡	…f'"?Ù[ì°s?Á™]Ð{ê?ã*óiH?ÁԚ´Õ<æ?¯Ý¸#ê¸=?œcñ~ùSj?☰ŸÖ±?¶M'TK?ÖÔAšBû—?µÂχ	?¯íeÿ¦Mc?¥÷a#p?Û¢· D?À+x1rœ]?à0ĞÍX?ÁVóïGîN?Š¤¶Ñ7
?šð8ÁûS?à·É[NŸ?фw^nÕ?Ý»HñÒÉ?ÑÀ"¨T%$?‹S)ȦL…?žÞ¢q¶Ný?Ü&
8€W²?¼ŽªÓ'Úº?ᬼ:õ?¾Ùˆ˜¦´?ïðâÅv[?ªy•ü­Å^?ßrbË€?´­ï¡›?Öµ¤Ã'R?³RBmº?³`‹›ít?§,Ð\h%?àg¨č?´çŔ9×i?ÚY§Èþ®i?·üvÀȨMIXED3FGL J0905.6-4917@pà
å6P¿öÀ³Nv…˜À8†î‰µöÇÀ:¸šs´-@"
¼õ@X‹{ô˜?û?‡ñ\?îê0õ/0^¿é=KR8Üë¿í<Ž"ER"¿ïþvì#1çUNASNone?¤âèªê?¦WUV'—?äõ"]*ä–?Ï`¥`þ.?Ӓèúª×?Ά=³â¥?L†O½fû?dþñfLù¢?ã›oqÛ£?Âk5"G±V?غÝöY§Ö?Âp,®à?Ãbb1È?¬¦³ûü?Þ¦ގ–0?¶–(ÁÙî?×Ë8ðXål?¸u«àpr?•Æ—Ù™ò?€à«  ?èÅ˦²÷?¾r¡?!ËN?Ê/þj©—?½ØííXÞ?˜æÝK€\?£…¨å«¯µ?ë´íJa3?ÁFÂã{ C?¼à*w¢Ï?À\¢ ‰?]âb=â?v¶
IáB?å'üàÌð?¹Bò¢R?Ô¾$-[ØÄ?¹]OTe­»?É·ÆZº-?±r]¹(?àªҌ?µM¿(-ø_?ÒþtIÓޏ?µW™t#Ì?£ÀA"½x?'î…*ãÁ?霭JP†?²¤™ÔíG?Ä|ãø¯Ì?°ÐEϸ¨PSR3FGL J0906.0-4705@pƖOv`?¸–º›¡À8²äǕUgÀ:}‹–¡—•?ù"Ÿ48@ä@,9—ÑB}?þÆÌÐ}±\?˳–áÈ ¿ê0";¥Œ[¿îøì»Þ±?§gji͛vUNASNone?Õ¡ḻôÚ?Ó5DŽ`?·˜CµÂ?½–Ç[‰/?â<F–¬;?҄˜vêÿ#?¸áþXe:Ð?Ãê·‡ÉÁ?°ð‹u<ä?¯«œ®§?êÅ®ƒi4*?ƍî"qX?ϳ$Öµ?#?´'ÿÏ!¨?Æ$zë{&?­u€ü
ý?âŠsîî?¸n¤GçX?Ù5pJüä©?ȼ~Ëâí?±U¥@²Eå?¼ÏÜ)i¹?á:"2]†?É_˜VxÄ?Ý¢épéÄ?Ó©~¾ø?ÀS»d«·e?Âׯíî?ÚÐd9:‰?ÑjÚgGÀg?ËÿÑ?‰i?ÒÂk±=?³«'‰K‡'?©	"ã®9?æŠËºAô†?Ñ°ú»¿Ö'?ßQ-ý*?·D
ÿz¨?Â$d›,Ž ?§m§ÊË?ל ›Q»Æ?¶YO`ª(¢?ã~Ú:…
?Áΐf•
i?°=ªvqÝy?°â®žÂ?ÔòàîÓîæ?Á¨sQ0t<MIXED3FGL J0907.0-4802@pӓ ٔ[¿Ú¥¬ÍSŠÀ8Ü滋[éÀ:›#ôÑΔ?úßÐVD/@
©¿³´£?ù2aŸb?ïÿ9†$¿ç×e¿èšg!¢<*¿ïÿ¢å8¿UNASNone?Œ#>äæJ×?'Ë@ےbn?ÎØ2Üv8?ÍU—}ï?çÙfM3[ï?ÍçÖÓá¾÷?EÚQ/¨X?a24y:Í?à¸åAì<1?Ä:ìÁ?ރHSÇ@?ÄF³bîaÈ?¹èÊâÅe-?¥€
<ÉþÊ?Ø}û"ˆý?µæ-3¨?àƒéAÜ?¸~@!Ù?šŒÝN?I¯%î?ã|Õ¸«K?ÀèI¤}'?×d«ÏçI?ÀÑ@é˜ú&?Ç›çOûƒ?¥ÒÝMb?×ò¤Î›?Ðv
øpXq?ãà ¢7?М™V†R?a¨[$P-Ë?£"gõ6?ã
h1Ü_×?¼3»÷ÅýX?ÙÁÞæĉv?¼ˆÉg½~{?ÊÿfÕ˜?®ºa
ç?Ùé«ð‰?"?²	¿
[<€?ؖ ¤êtl?³é³Q?|†?¥Éf'>Sæ?•ùWÑ?{«?ä~º…ûq?¶jlr~?ÔI^%صA?¶6Dac/@MIXED3FGL J0914.5-4736@pÜk;¸<ó?飺º{'qÀ8/·}°/À:žQY•@!!Ðà,Ñ@="àø(@÷(pa'ë¿ÓÜR>™ÌM¿ê"åʬa¿í(åÂŕ¿Ò?ÏezÐxUNASNone?àz?ºç-\?Í&Ä£C?ÄÁÆx8»?Å¢AøŒ²ð?Ôý¥â¨+?Í[¤æåä?Ð<sÃòÅ?Ò˺ «NÖ?¸`Z¤4~í?¸p¼	»S?äÕºÉ-õ ?ÒׯÔÄh?Û{³ÙЅ-?·Zõ܇ø)?ÉOó[4Œ­?°i˜b‰xi?×ÜRw'S¾?·	°þœ?Ö/Sƒò?ÂâÉ:"q.?ÇL9Îq¬Y?Ǝ¦r+QÏ?Þ*Rüs¥á?ÅR¿ö$´ë?ã´ÌqCu\?ÏùU…²JÚ?ÅÓjè´½?Çÿµ­K},?ËY´Ð	uÓ?É׬WiüÑ?Þn'‰&?×)o`Ç&V?¶l¹kôn?¶+›æm5L?Ûö´9$†??Ôº'÷Œ?à"ZÁÓ°¨?·SZaᡏ?ËÓ£?°ÙöfÈ7Ç?ÑÑxû`ÖQ?³€¿ÅîZ?à×ïYùµ?¾H)[æR?ÌâÇb!)¾?À;'Âpä€?Ͻ|dvïm?·¯yCMIXED3FGL J0915.8-5110@qÚ{9¿øMzÂ=ý'À8ÞfRDpÀ:ÏÍ"]"?ú•M8`D@õš9ý|Ã@a®‹™%Ö¿ÜzS®'ñ¿í ÙoP"‹¿êOÅóiĕ¿ÎõJ¤mªUNASNone	?Ѓ¢–Uô?ÅZ¤M#?ØÑ;$ ú?Ì\>
bë™?×eŒ.Չ?ÌrÃìÔT+?ÄÕì'¨\ø?Ì©oi^,J?Ã,¦JƼ?Á®É-ÓDX?åÿ[cd9¢?Î׸ËÁ"?Ü ¸>AÑ?µ˜ÛI5É?Êå—îbƒ?¯[âMïJq?Öv"O}–¯?·!åƒØH?Ô¸mÏ9u?ÄG
¼­¬?ËŠæ£b›?ÊnÍØüä?ݼMlß>?È÷~ôt?ØÁô¸_h¬?̋A§•/Ó?ÎØYfm—?Æ0M×	¢Ò?×Ñޕ³AG?Íd\ËÝäw?ÐÆ*"Ÿ?ÐásɌŒ§?Àï×m('3?»]Ҍ2"?ã½B*C?Мæ¡pcÑ?ä^¼GL"?³N «ct?Ńt'ø‡*?ª`/Ð6a?É$‹êHM?®Þ…D?ág>p(1"?À»©ˆhހ?ÌýÙ<ÐI?ÁKçKË|ã?Î]f"k1?¼¢V›\MIXED3FGL J0933.9-6232@q£Âã>ÿÀ"`úÛÀ9¾ÙÅÔÀ;" ¨ìó´@jl(T@RãKζ¿×ÎR8œ¿Õ™éº]"_?°ïÒq¿á¤"gÑK¿îÊW…*ªVUNASNone?ϕ'«
ç?Óûxîø?晧p$¼?Ôi9ªp¬?¨ƒ¼É°Ÿ?·	eÕ(V?''·u³™?¯éÞ,Oý?è>l{˜¥?ɯ–
тr?ÌÕ÷"¶¹:?Ç}A€º?¨I´¹a‰S?ã™BÞç?ë
"Iî¢?­bò]h"?»nƒZ+ßF?©K™ZªQ•?Ã4Ô*¯d?À,~é-ð?ç}õ£¨¾?ǘ8—1p¢?½¦ªŽ´cI?ÀR=ŽŸ?Ç%Ѽ±ÝÄ?ΪHéRê^?çñPì›c?Ðä:>a±î?²)Õ åE?Àâêvçú?¡›PØ#†Ý?¶ÕÁÁ؇S?è¹"Ÿ'<?ÅxÛüŒû?È´£bg ›?Á6O、?°â=-è-—?¢™×é÷°?êwÄS›Lf?¯FÀüÜuf?»_ 4Ï{º?ªðýDŠ?ȏçg€Ë?º¾²Q
?è-ՃÞ$?¿Jʇ*ß°?­†ŒlL"?°$)v 6ºPSR3FGL J0953.7-1510@o~"t¼@=šÿ}úâÀ9Ý8§z¢À;ùõ3c¾?üR:Ð5@
É))D?Û«g𲸭?èz;ì{z¿ÎOo -¿çnS	½C¿ïÿ¬r†§œUNASNone?'˜XÎcªé?!Ä Ã?ì.ôäæ@‰?Ʋ™Ì*¡¥?¹âB¢3h…?؏À8%?†o<lЊ]?¡7pà?íÒêF–xŽ?¼"³M
¾ž?­5Œ¯×?¹Œx‹tC?°®›bHSê? p¤"Ž'€?éî94ËT?²äÒ[ÅF?¿ß›^àò?®åÃSQ`Æ?¬'ƅ‰7?§´Áé×é?ìüÑ­ÎG?³(g)ê;?¤ã]
öX?¨ø˜›v?Î¸U?¡N Þ´
?ê'ù{ùÂñ?ÏyœL?ÚWmé˜?ÎPª|ë¸ö?™Î{ùu¢D?¨LZˆ£k?ìéæ0 .I?¾¤¶rF…?²=/€¡%)?¸ê8x?½‰ÍD}Á?¨ëžùC½?èá¦gw!?²ölXmÕF?½÷%Œ'±.?«öNJ'<®?Å|¢à?²!=2'©ï?éÈܵè?³ëjú»@µ?ž!Òªtm?¡g]JGœ®PSR3FGL J0954.8-3948@p݂ýuâ@&ê@1HwhÀ8¹}uv¤¢À;m2˜Ù€9?õËÔ.ÀÝ«@×-xß@a9n'Z¿ãÒ¼"Ëÿ¿èŸ"L±¡¿ä‹»S8óM¿ïÿ¢Gƛ¹UNASNone?Ý[E%=ô?ËHÐ1
ó?ÚiVö0ô?É#£§ ª?Àw_-É"/?¹–#§ÖÇm?¦´nêÀéð?°"Ѧ‡[?é">uÓä?ÂÕ¬d¢kû?ÅÉêm$NG?Á'N<gÔ?àî/aÜ-?µª`ê'?Ԟ"™¡Àô?²Ðn z<?Æ`5
d?ª‹béí	§?É% ­Áç
?°TÊq£'?å!ö?·v¬ÉeþÑ?ÂVa­?¯Ÿ3^³P?çhD'č?ÆXŒÖ_?͔wþ‹®?ijƒÌ9Q?£%Åè³Ü?¢
¥[ªÜÉ?¶V¸i* n?»¦Uó/?¼?èScô_ý…?Ä9Áh{З?ÇùÒ´?½7aý1TÈ?çÓ%ξ?°¡Xn?Èkâ†óNÂ?ªQ¡Aàsh?¶‰¡¿Åâª?Ÿê'ãûp,?Ú%î»xÖD?°Î±õÃ×?à—áâÍXþ?±ÔA'(7?²©5ûCëƒ?Ÿ‡Í½p²MIXED3FGL J1002.5-5709@q˜îcŠ	¿÷ƒÆÉ}À8kõœÏ®ÿÀ:O#
KB?öæä‹/s‹@œJ‹¿f]@Â@VÝ1?ÕÆ•^ ¿è	·}œ¿ê1øJ©òW¿êj_«rpUNASNone?Žˆ4êYÞ?–L‰ªêøý?֖Yˆ²k£?ÏðQG…?ä:²kÖ‡?Ð>‰£,jl?`ÎtRœ_?€Bõu¢?ßîí¼?ă´YREŒ?àeüºŒi—?ĕÖ!Þ?µàõó
? ƒY'<4?Òß±W»±?².l²­R8?ãÔ²Dúö?³;ñ«è÷\?""õi?‹#¡:ØW?ÛõHY¾•Û?À*ˆù¨ð?ádkÉôø‡?ÀS–Ϝ­?"®€á…Ï4?š¬àFœß"?ÔW>Wv?Ñx/3Î?偦б*Q?Ñvp4Eê?q'|™õZ?ˆš‡Ò¾
?ßØZ7až´?ÁØrïG?ßá_"/êv?ÂŽi é«?Çôt0©k?®%lÞ?Чç/y•B?¯õ=ÏÜ[<?á®ï\ڗ?´W(LM¬?Ÿò! ,¾w?"¿˜¯T?ÜBÔ
ŒT?´ op­Ž?àßc‰"2?¶oº'ZSOTHER3FGL J1013.6-5734@q°ò䎊¿íçù¾ÈR?À8€"¸aÀ:‡dK3'?ü»J}@9[‰"'?ù¯Àéz-?ïÿµÞ¯ßg¿è¹™ÈØ:X¿ëZ®ô¼Å¿äq[ˆ£
rUNASNone?ÃØÏØx…*?Èd¢ªBú?É]·žÅÜ?Ë>Ê~q}¤?äÃ4œƒž?ÐçE¾?'½aQ
'?¢""¾3D
?ϪC*՟?Ä÷ÃÛâil?çʃé¦n·?Å[…o	?Çf~À‹‡?±Ã²3"Õ?Ìé'ûr|Ÿ?²/ëC**?âëÿ'?¹'㛇?®¸¥¤D€?¤š¨neè?×·œ
Úpò?Çc4QZ)†?â8§ \E??ƬoÑ{ ?Ç;I;‹X?ÉßRq£?Ðḹ'Ô?Ίû¿¾Ø?â.<ÜTT@?ÑVb¬aa3?""/}…·›?¥In9í­/?Ó%ՙœk(?Äج×'B?åÈó·a`?ŝCx¶Ü1?×+¸ßžÐT?¶÷Eµ*"Š?ËÛÏ£Z§Z?°N3³™r?Úæ_N³Ûÿ?·=©UÒ¯
?¹6<Ê«?§2Ot¼¨X?ܑí.éo?¿Ô%'VÃ?Ý ƒÍCY
?¾¹ºmÆúGOTHER3FGL J1016.5-6034@qÐ=Ć­À	¶	8ÿ%À8¢qȚ8%À:í…AóÀW?ü4_,
@9ΛÙæ@U%o¦+"¿ÕðkhêáF¿íÞ[¦!šã¿è1Xh)'©¿ïþ°ð"g^UNASNone?±²´aZ'?°†œõÙ0i?ÝÜr	ä
?ÐSnáxð?ݶàÛç5È?ЬC`¹?rãg|»ÿ?'kÁ†Õí?åUÃY94Þ?Ù{Âoý?Õë¯n ¥?Ò×ßØ÷?˲p¦Â]C?¯•béhÁ?ÜF~àÁÝl?µööÒe?ÕàHËÜóó?·4håJ0Ì?«œã°Ì¹?™Kô¯;ø?æ»P)§Ýï?º$–"Õµ?Î+º «NÖ?¶äÞ¨¡²2?½%@v?¼¥¸?Qé?صdÁ\?Ìõ{âÏm'?àGBN%ŸC?Ð8 #È?ŽùQNÌø´? :æò(?å÷W¢©7Ç?À4ŒPÓ# ?Ó†/?ÄÍ?¿z¬Pwß?תóšR7?³§¬×™A?Ù5[¬
?²Ýå³T~þ?Ïm‹bŽ}?±É¢;x?ºJWÁ°J?Ÿ¬s7›|è?çÍòdÆ?°N•z=B]?ãÊÛÓG?§åߟ5°~MIXED3FGL J1026.2-5730@qÆM@$³>? µÐ±Þ´×À7Èn4'EÀ9þ¦-?ÿ¾‰öct@\è"ÿV?ü6ݲMD¬¿çƒ/NĀš¿Þ8I5[µ¿é®
Í{¦ó¿éE狏–UNASNone?gò°ïɇ?gW´!{??ã-ÆÔ)&Y?ÐÂ0o<,?ÙtŒö.V;?ÐØ(9sÙ?g‡Î½Ö q?z	%ÎÎP?Ù-ÌÕ8ߣ?Â]½AáÄ"?ãQ'Æ͕†?Âu7YÞm´?¤ìg!ñC.?•H˜Ä3U€?Ùv"–¨?¼Êê?ñª?â-/Rue)?½PÎ=U?œ9²Oß@Œ?–s–ˆi±Ð?Ûú"¨=BÎ?À원%æ?á ðFçµ?ÁU
W‹›ï?`ó2ÈmWG?e[';gâÎ?åã)éf8?Ð%'Ù‡'?ÔÅǨ~B?Ð;cÄ?"ˆÙ>õ?'Ì÷Ð	q?݂âp֊n?Àòä:É÷Ó?àình=?Á+üŽ—™ ?±9•pkx?¡ÆYðP#s?Û,¿qi?·ï½éŽF?àBmÅ>?¸]`÷²@¿?³ØpU8Ó?•Ç!)Téæ?à‰tqH?¸f¸]?ÝÚP¡‹´?¹Í&lƒêcMIXED3FGL J1035.7-6720@r&@·€4nÀPBÛÀ8`
z­EHÀ;?zF;†@'ð4ÛÕ@Í£ÈDŽŽ?ûôÆ/¿Ä€ó·áó¿àG±èDøX¿æۛÙS²ž¿îCRªò²eUNASNone?kR~ª»b?k¥¥ü1t?î'v"­:G?¯1¸Žm?¦#uèôÒy?®ˆá~tJ?^QÉ:4óì?'öÅpla™?êë>öÇo?¾òÑ÷·?Ä`'oŒ]?¾*VLµ1È?™îÕtáàM?ˆAÝÓ¬Ñ4?ì]l@+Ou?¦Ìõ—•_-?¶˜èŸµ>E?¤vØW".\?"eéÑ°ÛV?ƒ®Ö)ýà?í,‰èÃð¨?¡¨›}x?±'6C¼uð?ŸÎ®'\æ?Vj½»ÈO³?\wS•ž£G?ïzÐUÃ?"Åÿñ?Ý`?ŒìIŸO%?""\;WS?qIlÉ	?|ºÌƒÏ?ënØB½?·˜+úEË?Á¼]ž–®ƒ?·z­±"?¤rp»Íø¦?•ú}œ¤?섦™|á?¤K°›}oN?±¡—)§?Ÿ‹EFoËÌ?¨–IڞÚg?ŒŠ*k¹b?ì½ýÇÊ1?›ä›ök+È?«‰Ù­å‡?•'Çf¨ÎPSR3FGL J1037.2-6052@qõ"œwškÀT*#¿ùÀ9ûkEÉ8À:õå†6a?ø‡,å'?@
Ââm©Q?þ£ÐqÇîl¿Þ7 <$bO¿ëŒíîÒÓn¿áûÛxê«
¿ïÿÿ¬?…ôUNASNone?™eû a
P?§,LÇÖYC?ä³pí?ÈtXªÄ—Ó?ênæú9[Z?ÉK0h[;Ä?|¶í,Éñ?Þvº¾Ï«?áóú/l?Å0­Å©§?Û¥/ìÏ#?Å&aV{?ÐÙËc7ª?±:F‹ IÆ?×FÝC+g§?²ƒº3­?×àñq`¯?µy?/`ƒ?À [›˜]–?ªqß6žÝ?Üôþ4"òH?ÁüªçZþº?ÚúÓþÞí?¿Ù7z{ØO?µçíê/²k?¿Jâ/DÚ?Í´	¿=å`?Ðõ%pýÄ?åÕÿÒnÞk?Ò)bÒÄD?"ÎÚùHFd?£ª¬8?âÂ/ëÕü?¿nÍ'»…Ó?Ù>Õð¯L?¾,WKì<ª?Û44Íßi?²NA,uGã?ԇt¤¨Òƒ?¯Â™Wa?ÐD{&‰N?¯¡
ñˆ²?ÅûD™âê›?ªC7÷T?ã8¤a/?³·n<òÅG?Í"¼Ô˜Yd?¬îY*çÕÕMIXED3FGL J1037.9-5843@qåz–¼¿ÌèöÎþÖ4À8T=;"À:c?J˜ª†?ùhðÊ-
O@
Hy|î"?ü]Bf×пæ1QÚúHA¿äl(
Ôèìl†!Rò¿èJGy€
UNASNone?•ì
¸gPv?š]ÐüÃp¿?Êþ=¡åÝ?Çìý·ÙÔ%?èË ¸Ï%?ȸM—k»?i@Ým<o ?{Ê¢‰+4?Õnڏ÷?Ãĕf?%?å`‡µt>?ÃñgV%{?ÆΈ†TØ?­xaJÿŸá?Ñ_?òo"Ù?³P®aZk?᜽åB(]?¶A€÷uè›?¨†ð™?¡@‰KÝgé?Ø¡¸Ý'Ô?Â
–=æâÅ?â'"Àœ?Âsõn˜?°É9­ÿ?´ÔÖ"wSh?ÖT'e ?Ë;|û¾?â¼Öe°€?Ë£>$8c?‡ÔDâÉhˆ?˜îšÈ…Ï¿?×@p+Gh?‰¥·o(?䥴Úè™?Ãlø,]<W?׃ ҙ¦–?´®½T¸'Ê?β›ؼo?¯Oê‡ã?Ù#'©yû2?´¬—'ƒTò?°°M$]óÊ?£D3ÙÈÊ?Ý+Å·j÷?¹oª1í8?Þ¨'tïì?¼@8MhOTHER3FGL J1039.1-5809@qã4¢3œ?ÖuÌ}ɯÀ8ÖmpEã9À:x‹îN?ùžv*úÕ@ü²ÎHøÂ?÷'\ÆÕfú?ï՘KÌîA¿à'ß\¶(4¿æ£% Bb¿ïÿá…ÓiUNASNone?Mª²˜†…©?Vð*O'é%?ËóÿÁ–¹?Í+°²åÆ?é6˜S¯¸?Í#á,fv"?@ã΋©è"?Z™—a¢/?âtûu_[8?ÆhÀfj »?Û
—-ê°?Æo(=&b?¦I8fÐxç?•¸ž<¤?⻏VZæ½?·þ3]a?׿ºF¬Ê?¶½%hXÿ­?'3¬ÇËf?‰h;%Á%?ã±
"F)?Â]2užÎ?׊ªü¡y?ÂNìuWŸ?Q¯+2ÿøÆ?`–›+wφ?dž̞ß?ʜñ›P?ê3F·RÜ?ʯ!ËׯT?]ëš(óÜ·?w~wXì?ä	î‡Bæ?¾F)žÎ¦…?×Î7V¿Š?¾ƒë¿Mª¥?¼ëÒÌk(?¦
_Í»¢=?á^^ÁÆ"R?´¾Àz0?ÖMÊkÒ?´˜(‰VÃk?œ©6—,1?'SZ5¤©L?ãµ'Z?¹8â¨3ï?ØÚJÂN¢?¹'>ä
ÓMIXED3FGL J1047.3-6005@r½<64¿ë–eÒ°À8Yóv"Á›À:;°ÂF?øF&ñ}@$	-{8[?ü<|Ã$¿Þ®ØÑñW¿ÄòH'ú¿êÛÞLž` ¿ät+º²²´UNASNoneT?Š}ã4â´?‰¶üMeZð?ÕI^.o»5?Í%ýw†ì?äñY[æۗ?Í-äÝñt?'¢å1ml\?™&0Þr¦6?Í%2¬"?ÀÓ°ª
É?è)œ+ÍÁÈ?Á£B"AüØ?¾ÖßÆàµÉ?¦}ðܗ?ÏlQ?–L?³|ÿñœ?ä`òÔ´?µ"B
çUV?ºȆ']"?°^ëuÖÝ!?ÖÇܧO(¡?Ãe'
æÛ?áZ›
¬?Ã]½ÈDt?—›$ŽH»W?šM«oà¿?ÉÆCŠˆŠ?Æ،,¸^›?èѕùî?ǗØcÙÄ,?¥>dR?¯Ùq¥"¨?ϐRÐåê?ÀŒÖ6FÒ¼?æÊj·®Øp?ɉ³ô?Ìsz ,›??°3ÛûÜg?Í|þgh]Ñ?°ïŽõz?áƒáÞÁ¼?³ÁÕ|º¢?Á–?©Û}Œ?±%RRëÝ?×M­"Å–Å?¶n$fÍД?ßç2–Lªu?¹ûÝŒ–ôOTHER3FGL J1048.2-5928@qý³Ð|"¶¿Ð¬@$Þ0ÍÀ8Esvð!fÀ:7F°¾yM@…'5yß@¾ÅÍÿý§?úZ¢e›e?ïϯ??¨Y¿Öºèÿ]mÄ¿ëÊÿèƒ¿çoi¡H(}UNASNone?9V7ð?°u^U
?Ó¬ý‡ˆR¨?ÏE:^åW?å@‡qE^ü?Ðܝ‹|Ý?v	\ýá\œ?†'®A+à?Ô£˜S¦ú?ÄØî)z?åÇyûf
?Äü^fMøí?º·9Må¢B?§-w£ÎÇf?Òw8¼ñË?³2Ô{g/?ãm|w'Ò?µ<Ÿ'ˆ×u?£C±"8æä?¤†*Ӟ?â™{³÷á?Ç_èíX¢G?نVÕ¾|Â?Æ~Z–?¾Epô)Þ?ÃÇeYËù=?Êï«xX7?Ë>¿ÒØt?å{gf´6?Ï^[l¯£?‡JûC0@
?¡ÏR!Û¨û?ؼ×*Œ	?ÃxÃu¶œ?ãDh}þï›?Ä"ĝ©?ÀÙŠ«?«8¦>,×?Ö!…UՌ?²}ú1?à¾x¯êu?´ "Ç@¡?©
¯Fþ6ê?ªnª·áõ?ãøl(ÙNL?½FæXäóŠ?ÔíqÅ6¢Ì?ºŽb»F	MIXED3FGL J1056.7-5853@r	7ޓž®?粓€zä£À82Òò€»|À:°†ˆD݀@ð+Voù@š@QT?ýaÿI ÛB¿Éb_CF¿åÌ<>Ó-¿ëå­X_´é¿ïÿ¡Ïý6UNASNone?Ž,:ÿ,ò?'ÐÝ0OÝ?ã(£3Ýc?Îäëº×4?ؾ–àù÷Ë?δ_ºòý?4ðTOàD?ZˆWKo+?éÓ±s]£R?¹ã™J?ȦÂ0*ƒü?¹áÆ."'G?¶6[ï?¥ÖñK®Àw?âóq%ÔrU?¹/°a?ԋ†¸ã®2?¹A2)#ä?oNñÄÏÀ?fU—ŽŠóh?ìùƒgå'É?§J;'BÜ?·9m3/
|?¦½ÄéuòB?'àPý9wS?‹æy"Ë'?èÂÃDÉð?ÈÁüïä2?ÎvïãÀ,?ÈbÉTÐo?QT1s
?iy‹¡˜?ê#óèD¢q?°dÔÍ^ß?ÇM‡ûÀö?°dY햣?À˜ÿÅv0?ª¥{·¾?ãïT}v?´-nÝø&?Ï©¯âCú?²k'{(|?}¨_Þv";?mÃohË?í!½È€•?žˆ?aç<?µtlåÊc?)'Ò¾ªPSR3FGL J1104.9-6036@r#¹#¢œx¿ØæØ|-xÀ8脹7ÅÀ:~¤™@3gáe¶@l\õyi?øáY÷˜'?ïÿX"ò2¿Ü-vÕ8E¿æ
L|/{n¿ï~@ÝÀºñUNASNone?)>Dj È©?* 3Z[?âÞÊZy¶?Ñ¡îSýzŒ?Ú?C'
ܨ?Ñ¢DÔ¡?)~C7' ?O–â2)º?æ™$)]¤ÿ?À±§çSûo?Òʇ䡐ð?À±kžoÓ?‡§ ÅK=?'N‰Kµ
?æ÷ˏF?¼?¶ç<ʯË?ÑS/àËåÐ?¶¦ìlƒN?vŒ»œ2?q†öî <?æÀ	äôû"?¼f1\W?Ò'Ž¹H?¼T>×½Qì?çèl1Ó?¦ۘu?äTã"4ï\?Ñx§ \E?×UZƒì%?ц•…ã¯?@níƒV?cí9²³Ü?çî­âsI›?¶<&A BÝ?Ðm1º?à?¶Að§ê·'?ŽFBÁþ?‹C¥˜Á²†?çd-¼É?²ŸÉmš?ÐE±z‹âL?²3hK{¥ÿ?|!–ê›÷c?uR!ì×Ì?æ÷…êÝ{h?²Û"²¹v?Ñ mΏš'?²ëd…™:,PSR3FGL J1112.0-6135@r6^Ý)5¿î¨0 ±»ÏÀ7Ù³×2]À:C6nQs@«húp@Έc¼=?þ#ÉO"¾¿ÑåÅÊ­–¿æôþǛµ¿è]—ÆìÊ¿í£ç?·"UNASNone@?eé[O'J±?a'äLÞéz?Ü"8xä»?Ðh?áàý?áãÍÔ1g?Ðf±›Õ?M¶GÚ¦Þ:?gäÂå%ß½?ãð˜Gκ?¿ï"÷OØ?Ù¹C«Ùë¢?ÀLÌȁJ?¨°›ºÐ'?›Ùø'›.Ø?ܘÓL)	 ?¸Æ¿Ì(û?à(Œ¢K€?º~G·,Z/?"Ð}£=?†¾ãÏ`k?ãÐMhq6?¹%Rç+éU?×Ï]‹Ý€?¸öróÖ?W'¥ÑÚT?W&,ŒÀ`4?á.¶wS|2?И-ÐÀ×?݋kjԁ™?З ™=(?`-|øg?u˃šS{Ç?䤮/J<Ü?·oN#î?֖Ff–¸?·¦É "'Û?±0vKª?¢#·xÔ\v?àN<jr?µä4Ï=àù?Û±õ'F?¶Óö|g']?–»fÖ K•?ˆßùQ‹?æ™äKïm?¯CáÜGvß?Ñb	ÊÚl?¯Å©G*šMIXED3FGL J1119.9-2204@qGƒ[Õì@B†6`åÀ8Ώљ»(À;™tÆ{yô@$7÷E¨@Œgƒò¾N?ö
óxˆ'¿¥øV9]¿ß,âP–¿è Âb(‹¿ïÿê#¨YYUNASNone?"XôE´*š?ù> ËG?ìFu×êÚv?ęH
éUL?¸ö-"S©?ÃÅq'¤M–?¯~0¨+'?¬Ø9"È?홇à?Àc¿Ü/?®Âàw¿ù?»[|Ž­®?½µLE±m©?ª
‹W,NÍ?çôð4m?±¢\µpaR?ÁQ™ÌU"Ã?¬üå×%d?£$ºþY?–'m²3d?íϹ¬²?£üœDÛ‹?Ÿ¿V|vÐ?+ÊññÃ~?'éS+¦?þ?ŸÍTaJ*˜?ì[6nÉXÆ?Ė#´K\Ü?¸«÷À"L?ÄáhÂ{?Ÿä…OÔ?³Ê=­2ô6?ìÚ@ó\¥ë?ÂÊvîZ!?±4Õì®3?¹‡J4øk?¾°&Êçg?§¼
ÿ)Ä´?èhƒ³9?°Šƒm˜c?À^SÝͦ?©´ŽDTWk?¹FʔKA–?¡<ÉøÆ š?ì8&Ië±i?£\ÃÒâ—c?"àl5b?'ƒoýÈ©PSR3FGL J1120.6+0713@oqÝDU@NW´NPÅëÀ9ÒñÑsûÀ;åû¤P¬Á?úèE‰L‰@þEjÃB_?ñ›±‰¥ZÃ?ïKT
¡Í¿Þ~G˓R¿äH§Á¥|Q¿îÃËV€bUNASNone?ƐÑÄz»?ĘóÁÙ(Ñ?èƒ-(y"6?È¡åò§k®?­Œ¶4Ä}ª?²¾»…Pm?ÔsúC•	?ÑÎd;Íy?âÁäéú=?Òzp1sóö?¸ }p?·éBõl)ÿ?ȓ†¸žö?²ƒžÇjˆ?ãë筁`›?º·ß,")?Ǽڑ[‡?¶R:a?×¼_˜?—êíÊ?â0ºbðmÄ?¾³¨þ*W?¯áÔù?­v_[CîM?ÆБä­?Æ"maÇ	-?èæz®
Í?ÈÂ[Að?¦VC n¾?°þ^j±‰+?Ü||U™˜ ?Ñ"žœI—?ÞµÀû(?ÐÑP,ñ®6?³9£©²â?¯Á$ÚÈ?Ñ-ïZ?³`ؼQüã?âz~
¡ÿ?¶³­Îô‰?Ä«êÃDŽ?°ú†Ë4?ãûXôÁf?¹'&ӂ?Ö²À˜GEJ?·Ó7/
<l?•h×ïeŠ?™TÞ¢¹ÞMIXED3FGL J1128.6-5434@r0˜ñ/@z	Ì1œZÀ9eDܨâãÀ;cÚTtÌ[?÷9ÞóëË@
M¢÷Œ¿@
l…E¤¥¿á×i'òÛw¿ë+fiþ¿ïØڌï¿ïÂ
H½ÞóUNASNone?Ñ­ç°d›?Ë_;*^´}?Ö=!¬€¯›?˱÷¬?Øö£3É?Íå_€C1X?°Xù‹œ«È?¿4'±ž?äâŽå'ó‡?Ë`0ë
X?Ò$£Ñ‰} ?Çñ\c‡?ފ;hòîÜ?³7 قÁ?֎h™Ø"è?³¡êGS?ÅηüŽ¹õ?¦ƒb€À¿)?©vŽ´…¥"?¢.,1µ?돁"=֔?¶Æùà<|n?¶È¬ƒÎx–?°×Gmi`?׌láïc?ÎÍB¢€·º?ևB"g?C?Ê~Ø/Üß?Ñì ÿ¶ÑZ?ÐÃjûn?Å>|Ê4?Éxµàïeö?⽚™ˆ?ÊMqÚ°1®?Ьêü…?Â8*uÁÅ?å
šÎ«|Ï?¯ZÍeà?Ï	8-C7?ªË9ét'?¹˜¹0?ž°ª…¹¹?ÅÛ5 ‡?­>Ì.hÍ?è(eZ*v?³Í¼Sž[Í?³ÐÀi•…?£›Ô½t#ÅMIXED3FGL J1128.7-6232@rYŸ±¿òÓe7'=…À8º5À¬-À:¶î#;n?ûó"vøYî@|CÐd[õ?ù!֙Õ(¼?ïô`9¦"Õ¿è:5+Âå¿êg…î
‡¿åáe<3¦ºUNASNone?¸¶¨¬LÑ?¶&*؍ù'?Ñ<®8(e?Ë<БŽ™r?äJÓù;ë"?ÍhñƁY1?€8¹ô9?™¶ãu
?Ñ^â…é	?Ä­pUÂC?ç®z7Ê?ÅCûùê?ÒéüÉûÈI?·ßŠ	pÒ?Ì(1ô?³AÞUÐÿ?ßow½¯?¿îßú¯'?²(`€b)Û?¤Êk•ý?ÛP¡6૖?ƞÈ
±½?à£TÈ)?Ł®Ý3Þe?ρ݁61¦?È<N|‡1"?ӆÛ@Øã1?ÊŽªA v?ܸ5þŒü?˸«Ô'y?›k×	SË5?°Ô:ZÕõ§?Ôe‰(·7?ÃÒGX²/?äñÜÅ×ÿË?Å0Ì=R=\?Ý¥P¾½H?¸…!0Š?ËÝdn-sð?°\ß%L½?Ôký¹¨?·dûú—Y?¿ÏþõM?©…ƨñPe?ߜû3¥D?½sd2¦è¯?Øo>Ž}~'?ºê¹²=ÕNMIXED3FGL J1208.4-6239@r ]'ýuâ¿É¿{*˜°À8ô!-wÀ:	÷;5`4?üJ5XQ@©·6ì%?ö̼†®…d?éòz1Ìß¿ÖÀ}xü–¿å®€Rî¿í§õ'ùoUNASNone?N¥A'Ú'?Q›¶/¡‹/?ã¬Þ1;?Ð9¦Ý?ؖñF‡V?Ð_žÌ'?eÜóâÊ«?x8¤6U§|?غØú¾³Á?Äv""?㌶Ž¿Bm?ÄA´!҅? H`³G`T?•a»ç?â/Þ]  ?ºfß7ó?ٗ7/¨Js?º ¢{¯<³?¢j&$"?š™V õ£C?Ù$w%çd?Á
I\4½?âG"v3l?ÁªÑ=q?X°ŸƒŠ,?eÅÞáÞf?âZT?u'?Ñ£#?Û2¹Ñ'³?Ñ	½½Ý"?yQó®á?V·?ߤÙI™g?À!¨[Ô<-?ßöínû,Ô?À§i3}ä?°%g+u^?¡®Ñ·ˆ»ý?âÃo^7?¶©ŠHò}?×ó4‡"?µš{</‡â?¦§˜Ï‰Ž? Û$Ík€?ُ/3ø;?·${¥áÓ$?áÍîñms©?¹<E7ãMIXED3FGL J1225.9+2953@g$ÞÊl @Tðñ¾ôœõÀ9wÒ4jkÀ;¨Öí·ÿ?úOó«³Í@>¥"8äù?óJCðð™?ÒïXæ© U¿àW¼ãÜÄù¿×UXÂ8õ¿ì'ŠyÉ£*UNASNone?¯XS©ûZ?±Ë±ŸUãe?ìӚPª?¹Ç¼JQ:Ž?£nV¡Òl?­‰>CçÉC?ÒG7‰´?ÒÁvCƒ¸?áêz)3M?Ô~4mÛ¶?ÇYçè\f?Ϋ§®ZEò?À]«GÓ—?©€šŽ?èa†¦³ï—?¯¨ù8üæ?¼8t:ºf?¤î¢"€¬?Ù­"šB?Ã
þ×r(x?à†Ÿ×Ø?Åmô­ÄýS?·œÆv
ѹ?®»LLØÍk?¸B¹Ó&×P?½)wˆ!Í?ëƒË•Poë?ÁÌ_——?§=Óî¨?¯ˆ¿óô¤š?Û0ÑóÂ?ÓãÚ
'?ܟî˂Ób?ÑÓÃ#Õ%?À›ê	|35?ÆÂ}9Lãð?ÌH"ÀoNö?±lR
]k?å8ÉxëŠc?³Cèø|~?½¨Œ³y‹ÿ?¥ïÐê¶<?á#»ŠÉáÐ?¸¯@¸S"g?ÛÚÕ³-Î?¹-ÈKnú?Û3|`!?"Ëþ×ȳMIXED3FGL J1231.6-5113@r¼Aò×s@'»%}À9fƒÂ—ÀÀ;uëGWL?ûšÄÒW{<@ĂLuúX@ó¡­k¿Õ:æÄ*ù¿èAܕ†~N¿ï礉·¤G¿ïØ¡—>ö`UNASNone?»¾-ˆàu?ÀZO¡þÂé?ꌭv?ÃïHbDmÃ?´ÄÍmSÞ?µ"¸<!7?—M͏ûê?­ÍØà]K«?ë£Ü0S?¿tSé%í?ÀÛ¹ÄÝ?6?¼W[ϒ,›?ÕgŽS.??±ÿ~³ù¼ü?ß~òë*Â?´2YÒ*ðõ?Æ2ý…s¿7?«¦^ÿãÒ,?¢oJ«=é—?•œˆ4¸¥?ìÞ¶³t¥Þ?¬0ªt?¯¥J/††?¥™þ;¬>è?ËõSmÃÛ?ÇÝî—;µ'?ç!^bÈ|?ÈÕ6?y‰ü?®ä…ÈxÍ?°ôɄݏ?­({zBèè?®ÿNëz«Ð?é'ƒ×C&?¾±"ˆ|L?ÂqgmKï?»_|¸ôcü?ݲ¡L$œ?³©¨úBxa?Ù¤j®–ù?²+¢ëì?ÁQ£
ˆÖ?§ÈÀ½c½?À×4ÜÍî,?¢H?õ8{Ç?ê!8wH?§º±/L¾?«ÁZ¹Ç?˜3:yqMIXED3FGL J1306.4-6043@sKœ¶"Œ@±]''À8xÅ
»ªÀ:¶…F%~??ÿƒ>ùºì{@™;³4uS?õrjùs¿º¯&&bóÉ¿Ößë}ù¿àì6GöÊÞ¿ësiø¥²UNASNone?unH²ŸB²?– úÃ?ïëy¶$j?¦<Ôï÷ma?™æþ£ÊÐ?¤Þ=Gëk?OþýíV??b±u8%]J?éCö®À?ÀEÝH´¾?˞ô¨ÅÜ?À£»}çY?©3¤…üpä?œ@SÙÑ*?èÆ.Åæ(¾?°êÆëˆåò?ƚ[Ǎ.
?¬Êjà5Å?¯Œ]¾D?'Mf!1|ô?é5:èU·?µ$'ýÈa?ÉNҜ«­ÿ?´¬jBGW?aŠ1*E'?qKBŒU-?ï5ˆ"}iÒ?¦æj´?—+(ù ?¥CAŸçÏM?j0‰¤ÊËN?xvŽ¶Ád?ê>º…?µ}ù!‹ãE?ÇZìà"~"?µjÄM…"?¶ÜXµ
?¤ÇïšV?眼Xl?°öPVצ?Æá¾1ºž?¬zªí´5î?–¬ªÊ97?"%ÿ'ñÁ8?ê}ïšH?«_Ê1eHq?Ä´…
š¶?ª³ŒÆã®ÛPSR3FGL J1317.6-6315@sñ¾ôœõ¿á3Ïp;ÑÀ8?M«"}©À:g"©GŒ‡?ù9í|o½'@a'ÇMµ?ûJ)©ò'>?ïêu^üº¦¿ã^,æ#é¿è&lX÷F¿îgùt±¾æUNASNone?‡ÓSâpÇ?ŠP2è‹?äk!;Ž÷T?Ðõƒ$b5?Ök"ê!¿?ω]ÆH"?K2:]2Â?d?"U1Ü+?Þ¶"•>?ؘ—;?àéó¬¾?éñfÆCØ?¥þæ½sDo?•Jºéis^?áa:»ùÑú?¸ÿ¬é??Ú}­°&ù¿?¸ÿ¿[}²¼?œ˜¨Ýù'Æ?'Pg\‡?áZ¥3fðá?Àê%qÃU™?ہ+¥a?À™Ÿ_š?"åôМÇ?œñK«PÛx?è÷Z¥›Ž?Æ¥´|kWß?É¥ÖÏì"9?Åst¨ž<?dO0NZð?}mÝÁxC%?áóqÐ/‹?½_j-?Ûñ<¼&"ó?½âæ˜ê‹é?Áà´¶´?©Ú®mÙOÒ?ß[ÓõNåÛ?µÿ]Ñhÿ?×´#±h Ü?µk§ê
|?ª:QZq®?™¸ä@)?àkZþŸ?¶Õ¥¤ÄäÚ?ܙÿ3§L?¶¦È›Ù'MIXED3FGL J1329.8-6109@s8ҝÇ%Ä?õÕ`IôÀ8ÔG'‡|À:€ŠÔÚ¸?øBw÷]o@Åßó›?÷pµµ.£¿Gctö/¿ÝÓÙ"à¿âõ‡›D¿î¼P3°AãUNASNone?ƒ"‰×Ϟ/?‡M$,!t"?à(l)ì/
?Ñn›>4n?ß],«Û?ёžt0Í?™_teʹ?®U i™+?ـۂGBŠ?Ä	ÖÏä?âs'CT­E?Ås
	k×?¿¢'BÝA±?©`º!pà_?âÇ?"$Î?·°®qãŠ8?҈àIyø?´\31°§'?ÆbB'?°Ç¸ ¹×#?ÚÐîb§G¶?½!>Ýž?Ùþ|W$»?½$&ê"LÂ?":jÁHƒ?›ìI¢ˆ?à"7m].7?Ñ(út¼å?ݓêxYX?ÑszÉÓPÓ?±U¡ ûÂì?·0Y
Ë5A?ދµ½‰m?À0*ÞpI?ÝáÛ/n¶?Â7w_ æ™?Ñ5o`é'n?¯þ[‰?c«?àS…5‰y¼?²'‹3Æ?ÌGh5?¯º0ÐÈÔ?Îò"Ô?°ú–g«¢ë?ßm…'¶S?´z´º¬?Ñå0"=+?± ú6‰ëMIXED3FGL J1350.4-6224@s[ZîcŠ¿Ôy4¿zSÙÀ8i1ÈÏè
À:sî,ëñ?ý"£'–Æ@B%±ŽX?çµçF[ë?ïúT\ü¿Ñ¿•_V¿â"°õ·¿ïÿò|ðÒ¢UNASNone?aØõ1^ƒ?o>$GñÒß?äìñ³" ?ÒBèUr?Öj®I©í?ÒB\/ož?VXEd®Ã\?qÍIl?àëù҃4?É¥l…(7F?ßÁÏÆÚÍõ?ɲ"miT?¥üöÃj?˜0½"ó6?äåúwÍ8z?¶*bNu?ӐKÙ-??µ%B;¨'?¦iéù? ='R-?á§ÖЩ¼?Ɔ'
"pÃ?Ùã0AøY)?ÆI ŠB?[7Å÷?wIø=?š?æ"d¸ü‹?Ҕë?å¯X?Ó /> ¾?ғ•ÑŒN?jÙ· yŠk?"¥
òêq7?ãÒ†¸/?Áü9üûú?؎¨W€"-?ÂlZ@?¯ô)cßô?¡1)sºäw?å×"@r?³Ùb61é}?ÐS6—Ûm=?²wˆw³?Þ?­Ÿö˜Î?¡§íe>?âµòÞã?¿óbùb?ÖóÿØ#(_?À³PCÔPSR3FGL J1358.5-6025@sr	ԕ+?õè|4gÀ7䐴Ê!À:Sýå¶?ûI"dvL8@Éf<J7@Çþ†Ù#¿ÒVƒ¾Õ­
¿ä˜Ñ1$T¿è'&›É¿ï-9†ßW¿UNASNone?j£#š´­¹?uÛîˆ]x?ê²¢}±B?Æ1ÝT¦ÂÄ?ÄÊëgn'?Æ9^'ÔÑ?jmÖÀ<*ß?z1jj'Õ?ã@¤"+?ÂAQï`öe?ÙJé
£¥•?ÂM8ܯ1Ë?«7'Ófl?œ•ac½?ã¹æj–x?¶—(ZÑ®?Õ(lF`rÃ?µ"B+:ð?™¬aî´ç?‹àzš%?ãW@ÿ¤?¶tžø<ã?×·^Íñ?¶rD6?öô?uµêú‰šZ?†ˆ
y<\?é™üºó}Þ?Ë|£Ip·M?Èê]»`Øw?Ëa;ø1]#?‡ä"a²?'FMÇRT?åwTk£M^?¸÷£ÜóÉV?ÔR2Œðø?¹¦û_æ?»€«È…?¥àZ÷‡y?áÏCJ55õ?³í
$~?ՁN¦£´?²Äð0y?¥½2P	WÃ?•ÄvYQ?âî"0ñ(f?®"(yêÔT?×lT"=?¯wÌ÷PSR3FGL J1405.4-6119@s{!Bp?ҕa¼­žÀ7Ґ[,À9Ëp£×
=?ÿñ´â@BüŒX'?þ_ÛÛ£
¿Ó‹
9ÏYš¿ä]ï֫⋿çvº 5¦;¿ç"vµû
^UNASNone?]ƒœ,ö?b &^¸ý?»ê:¸dq?½|YF1+‹?ìt4¼Ó?½¯ùdQی?Tk4WØ}?xcõ…1Ô?ß|õôäC?ēD霙Ý?à7O'Ò¶N?ĉ#Vé"$?¥û;¹Ï?—¾ä¤&\Ø?ÌOxÙZ¤¼?²';µÆ?çŒn?¤?²Ëԑ"{?ƒ~;¥
Ä?€oñùÛºX?ÙRŠL°Ä?½röJR<A?ã+ÝÎt9/?¾yæ\&?RW‰ø@Â?Vç¤-.G?ÄƾàûØÔ?ŇáëíÏQ?êÅ$ƒ(O;?ś•Cñã?tŽC˗?‡Ö&H?â²#yèàe?À4†Íí'?ÚKP¡ê1H?À$Óôß:Ž?®1½'Ñð? ŸVP|kÍ?ÑÚ"ãQ@?²A[Ήš±?å/Ò¶E̾?³€Ï ^&H?†kÔÈ~?'Ùk"Èþ?Ú¤ÉÿÏà?·ÿKuÛ_ž?âUyT]Wý?¹Eb&9kMIXED3FGL J1411.8-5743@s˜•1ã¨@èX¡ÅgÀ8õil«$À;Î70ö?øº¢OÎ@'9"áV@áÈ¿Ì߿ŧä•o¿ë·Ö¡-¿æ[8'R3¿é†¤9ä/óUNASNone?»3LÄåß?µµêµ4
?Þ³€íȒM?ÌjòùB‡Ë?Úº}óS}?Ì%\g×L$?¸›˜"PUç?Â÷bŸ?ՐHNÅ­@?Ä?³5ïG˜?â$hÓå+$?ÉOB]r¢?Ú~¨²;Q?´AñRmT$?Ó‹ÓÄsô?³nÎçE?ÒiËz:ý?²€"û3ç?ǖÕî½?¯(¬È?ÞYŠž1·f?ÀÑ#}3?ÕÛhYcQ<?¹Iø¬¸Ñ?Ðe–tm‡?ŋÝ4_>e?àGhš{ÊY?Ê(*Vߋ?Î0­5Ç|?ÃÇÛKj·"?Ð\ú%Jz?ÐNl˖}?ÕL±8òÕ?Ðÿ25î`?ÚVT¡~%±?ÉÍ÷úÍæþ?äp…뀰Ù?±ð'ü¢'?Ë"j)áÈ?¬c%f²_»?Ã1céùP?¦à*ùX?ӂÂA–g?­³'"ò´Ì?àÕPÎhr?³×Fˆ±‡%?Å¥8¯Û
¹?¤wë¤ìMIXED3FGL J1412.3-6635@sm¹à`þHÀê°]*}'À9†ŽVox^À;@ï›2÷?÷U¸ìp+6@ò©nοÁ?ú2IÂ°¿Ýy¶rËØ¿âi·š›¿åœ0õì*á¿ïÿéåèUNASNone?·ÂB"ÇÀí?¸ íry?äÑ[&í*?Íëp‡»?Ǫ̀d¸'?ËkôI,]›?©uT?t?±õiI?áðM3Ô1µ?Å	•J>?Øð³­}7t?Ä^0:_?ÎÿáŸö2ª?²!''Íó?áÞ4X½3?µ@l«Êª¦?ɇLÿ¦Ø‹?¬ößè)ìÛ?ɐkàSá?±Ñ…Ç"N?ác½n'a?½'Ƴq?ÐpO2îï?¶Ö#V<Þ?Æòñd0×
?Ä®"—¦¶?á½îרaÍ?ÌÆæEÍG?Ñ
©ž–Ðß?È¡ÁàykÁ?ÄÊ,êâû?ÃDl'?àsú"—bn?Ã2KÑ(•å?Ô²ô`±èè?ÀEcgê†,?ßëñ•®þ[?²Tå"iº÷?×ræ'ï×?°íý-™"‡?ÁBO°ÂU%?¤D‰—¤ê?ԇ2䕟?°•Somêø?á[½–?²à\–E?GŠÇÞj?§A±ûýYMIXED3FGL J1447.3-5800@sÜï4Ö¡b?÷®ITèRÀ7ÿö¶«"XÀ:…Ћž.T?÷¢!Ódk@'
t­@Ýë´½·¿ã€ÌÝØ|¿éy<˜üT"¿ëøcb"¹z¿ê¹ËÌ$cëUNASNone?«@(9/!?°^mñ`…?Õ;žê"ý?̂)¹?"Ù?ã°¬ûB£`?ÎbOØ|Э?¥ØãFæã?´ÚÜöÐ&?Ù\óë
™_?ÅÛw"HF?âÈ|RƒR?ƼŽ¢Uæù?Ç&Gõip?°·¦~Õ)/?ÕéÆzÃî?¶'·Ü"…?ރk‡Z?¸™k‡ž«?¯A @C:]?ž3ëâ32Õ?àTßä›?¾ì=§¶Ã?Ûo¯ÆÕ¾?¼ÛO6Ÿ?Á"˜é	]?ÂpôŸNºM?Õµøû j?˙¼g'xÉ?àÜúH-t?Ð|1e?£=–sí?É@o¬5S?ÙWA•vŸD?Ãs,äJÓõ?ÝWæ>&Æ?ŶûGg%\?Þ×ÍSQÙ?¶Rè\l´×?Îþﲈ†?°«¢RO?Òz°Yhjç?²ÉH'׉Š?¿|ëŸ1d?¤XËô	Ғ?ß+°DMYG?²Ä²v0Ì?ØõÓæ`a?²ÑSm†MIXED3FGL J1456.7-6046@sÚVlô!¿ø˜}õÏ$–À8I)B©DÀ:.^¸<?ûCç@ìY@"óoMì@'åÆmã¿Ãö'àªáQ¿ë^}õàS¿ì"f›YQ¿ì17î-ð~UNASNone?kò:Äí?pŖj?¯Ý?á´c¹°1Ù?Ñ}³ßëãh?Ü_T‹:d?Ñz
jÕ>"?"Ѻ–k??©Œ5y{Å]?ڟóãšÑ?Ƃôš#à¸?âx:Ð]?Ç}uâlv?¶Üáz=d¹?¢ãp‹Ô?ØΟû?´1Ê5?hP?à½C6"?µJ.þšñ?ó•î§-¥?–®´f'°?×Ö]•îzƒ?Âr°@úñù?ã%4…¡GÁ?'ÞwD?V«e]úŸ?^Ú¨ºï3»?Þ«E+?ÓdÅb±aH?àŸ J^"+?Óe_Ù.…?¢‹Ô#Íz?µˆVœ·Õ?ÚÓNµßdC?Ã5Nš±‹m?ám›bá:‡?ÄàrÑ®³Ý?çí(?§ÄÍo¢	?×R†ßúý?²Kõàúþ¥?ß,¦W©Eo?³RþY֘Ð?¤Y'?œ€ˆ
›˜#?Ûi¥0â²#?¹ºÔ¨Êu?ášõ fÎ?»o…"XnMIXED3FGL J1503.5-5801@sûX£/D'?Þ7_úfŽÀ8–—†™ãÀ:5œBÁE°?ù§œSÞ#Œ@Øٗ
ž?þH»eqHî¿Úù> #Ìc¿æòn-@f¿æ¯'ùš¾»¿îڌ{×oqUNASNone?ˆî²û•b'?‡ññ;Cë?½Óa³ÆŽ?¾Èpßç?ëøjÈéÕ?¿œ´8"ӌ?'ì,Òޗ?"®(
Ï×?Ñ҉ Ѕ?¾ÎÚîùr?æыˆaq?¿™êLB?ÀÖjmº¡/?ªŒÒñ0?ÔDjÑ3S?µ³{M®Rœ?á¨0^¨¾?¸=TAD¤?¸Ç:"¯?ªÜ÷¬
S?ҝ'z?¶ßœ8ý…?ãäÐmÚè³?»q{S™–P?•éŒ²hc?™ùÓÐ~?»Ð"e°?¾«"…ó
m?ëÖ£sÉ6¦?Àm¾+kµþ?š«›6Ã.À?¦#z‰'!?ت‹M•Mô?¹3J"û?âÕ]Œþ?½°ËºS#?Î
J*ñpE?°kXdÄE'?Ò)Þ®ª*"?±á"P£?ÞÏ|<ïþ?µÍuǶ?¿}DR¯B?®;vԖÇb?ØS
{Pz¹?±›Wjí?ßͤpÀv?´˜3°¢ïOTHER3FGL J1528.3-5836@t"»â.]á¿û"à¢l¦òÀ9~e`¬éÀ;_Þ+™á¾?ý}©^2»>@ë.QL#¿ã–/—ÐÊ;¿Ö؎ŠO'R¿¤ëÄüÍ/C¿æ!ڛB¿ïÿÇí%CUNASNone?áýºÇ?وÓsÙA?ÑGÑó½?Ô:Ô6 j?Å؈?²¦?Ï
¬lkI`?|ýŽ?·\UØñë?ßËR7Ê
"?ÐÖØ3³5Í?Þd<Ë®ó?Ðè+Çâ‹?Ãó¬rí»ã?®"½}(¾ž?âëK?¼ï9øãðÅ?Ð/'«O	å?½W±Ï'Ç:?˒rG?Ƽk&zÏ:?âŸx°Ø?Ïk¦à1·?Éïÿ%~X?ÉaB°SÅO?åÇ6#ÂA?ØÐ/°û=¬?ÈÜqzÁ'1?Ó"¼é'?Ãq¬¯dÌ?Ά=bGY?¯"b‰Ü?ÜևX?àÿäl¯3g?Ì1AòÏÑö?Ú
ÕYýç?̆êhFÃç?ƼŸ‰ƒÞ?®µ¤˜q?âõFú:n?¹Ò£À'ç"?ÍoZ"8E?¹Àr$Ï\
?Ó	ôþù?Ãmߚëå?áÖ÷ùKZò?ŝDq҈×?Á¥ì	WÃ?Áï¾áŸMIXED3FGL J1539.2-3324@u,%ãS÷Ï@1ˆÁDŽPÀ9.èŒEôÀ;š^x[[p@(Ò·rrŽ@;«Ò(+¿ó…¦÷ú"?ïþ°Q/â?ç¡eº]Î+¿Ü>S"ø䔿í‰ÕB€òÈUNASNone?ÓI-½ÊÉ?×=¦C¡?å'2)€à?×Cqˆ7?•å*éBY?°%8†?"lvó<Ó?³ÏJÐÒ££?ì–X)•XJ?Ä>Ý´.Mú?¶ˆ£"¼‡}?ÀƒQn1¶Ü?³h±É€?¤yŸì(?韎_c4?³Œ2&¦"z?¿šÝ;"æY?²\.êy0?³É*¤ðð?¸[(nkêö?ëÄp¯|ü?ºDO÷J`?­‡b¼6_?·"5+¤×7?ӗi@éݲ?Õ¬'ìG-?äê³&¶Î?Öµ
_ÜV?¤™"ú""?ºpɅ‰["?¡ûûR`
ö?¿xGØdc5?ì8S(ϊ ?ŖQ#ÙË?µ?i-â‰?¼Ibªù?·>£käÜa?§c´Ï7ݨ?èç´Y¹YÓ?³ã×dÖC?ÀÁÜâLCƒ?±ëèäl?¼¨JƒÔ,à?¶PZ-cŠ?ë[b"ã?¼§çÚDã?¥™´Ë½òÙ?¯÷GÙ4C'PSR3FGL J1543.5-0244@K¯'9*Ä@Cs7âÅ\–À9ÀÁœ¬tÀ;¬U^f?ö|»WYƒ)@±¦˜/·(?þG;N	οҙÎeܱO¿âÞÓüýþ¿ëù+'Lm¿ïÿ¨×¥ýUNASNone?çrº`þ6k?Æò¿¶Êé?Ï–Žø*ô?Æß«Ð퇜?˜ÓÿoWñ?—8ëŸnò[?Þ·'e'?ɛ[½ÑC?Úއùøú?ÉÝ!êǚÅ?¹§kzˆ˜|?¶k&}bïH?à#ã±.¥t?ºâ£RëM?Øåi¤'øÄ?¹ÀkÍOöÛ?»K;ß÷nX?¤Õ¤Ÿïå?Óó2â–ì?¸]'èù'Î?âý»V'Ä?¾~ž|¾}»?¸G(#›Ì¶?ª×ÖDzé?ìΎ¾tDu?¹_T²¤]?·"xˆËí´?¸àÅ<µ'ô??þ!ø?~›<.?çâAåÂUê?Å.`‡÷}?É|b(`"¶?Ã!!Éåwû?«êXþ越?©ÕÔÁ	‹t?åÕ%ï:?±##&?ÎéO¶óË?®Þ¡"ói/?³"4‰àÄ?Ÿ•Â"p²0?ã'‡ý?°–íÖë[D?Öí~¦¬°*?°)®È¿qÑ?¦#õ™*Ñ?–ø>ÎC…ÁMIXED3FGL J1552.8-5330@t]$žDú?ÓkM
ìÓÀ7å-c™ÑÀ9ùt,!Æú?ÿþnÞ,µ@´Š­B˜×?óÕ7‡€½U?ïÿŠºZH¿Û+4*©ø¿ã¯wuhž
¿ïò]΃AUNASNone@?7}Õʲ0?EMró©?çöƒ´å™?͋O‰«
?Ð
7÷ú3I?͊(œp't?5n}Ãƅ?S›Ëƽ7?äg?šϤ?ÄÿÞ$Áˆÿ?×,?ðA,V?Ž­¨¢Õ?ŒQ1rF?"ͽWJÕ?å'ˆ0Ä!?¸Ÿï,ÊÛ?Ô÷êelží?¸[Ü	U¿$?Ãӆ$ÉÅ?}yQ†u÷?áÌ­l#-›?Ã/a;&E?Û؆Š¯W,?ÃL~¢Œ N?'ß‹aâ?)Øxþï<?ç¡›Lø?Ð3æá9Û?лú›ÖÏt?Ð3tËrÉe?Nû'dû…?lmPô ?ç}v½"?¸çF'-9?ÑÁ‡JrÑ?¸òƒO1>Ý?ŠúÑf_‡?ˆÄº¸*ÜÖ?嬅'qNn?µXÉPp¤¼?ÓÏRÈÇ&?µB¢È߆?ƒÀ•FLºI?'Ek	²]?âsöóÍþ·?º1B=ùF?Úz
n
àÏ?º¦æ7›¼xPSR3FGL J1557.0-4225@túB¤TÞ@ ¹mmÁ¤{À8ÔÔ{øÀ;
Ìhù¾?÷ÇV%{˜@þý~Ԝ@HåY‹Œ'¿ä Ä+q%¿ë[4aº
¿èM9Þaä¿ïÿT,ÉFUNASNone?Ú£òÛK¸?Èaúë\ô'?Ó1þÇ+?ÆÏ´fW+?Ò*$­€Ï?Éˋ ô$?² H^üUJ?¸ãO«Ëh?æPe`às%?ÆðåRL ?ÍnFLÉ?IJE²`T?ÛO=æÛí?µÔI§Øi?Ô»ã¡á¢Ù?³B†ïœ%?Ï龈ou?²`p¨ëŽ\?·³q¢¬(?¡³JˤZr?åîº#c¹?¶àèòc?Ìk—8ý]Ê?²Ôãã
?ãšf{½™1?ÈR¨8ÃÀà?Ì#¼#B‹|?ÁCEYÑW¡?År©íÇÁ?ė³I,o?ÃØÚP‡Æ¢?À³
2LÈ?ät
Ò£ã?ÂÈ'V[+u?ÊVúfý©Ó?À
‡"¹ ?äî€iFë?±d%ú¦?ËҁWè?ªoåþ±}?Á'»};Œj?¥"ÌÍ+J?Èٍ{À?¥èÝ-$øÉ?ä÷L¸ëD?¯åvøëõÃ?ÃIð?~×2?¢çµ¶¤MIXED3FGL J1601.9+2306@CDÙê¦Ò@Gx($xÀ:_ñ÷ÿ€~À<@žReþb?÷6(¦I€@ÎÝћ¿¿Ûäúr™Çß¿èÅ&õ?Îkƒb0ÝÕ¿çD uRº¿ïûõú KUNASNone?äaúÊ'?×wa[Äi?ÔX¦Jé™?Õրk[~è?§,âNMÈ?½¾ùá"?¾‹Ô½¡?Ì÷™3î#?èÅЍæKé?Ьzãöà?´Tcæäú?º­0Ð,}·?ÒX|HOúê?¸g°3&,–?ãWŸ[¥m7?ºêLí÷óJ?»á"ªœ?¦Þ.H7³=?Òkj·ƒåR?Ëw¾±Ԙ?å'˜M¶?Í4¾$µ¹?£" Å½|?¯$6‹ÅU?ä肟Ï`?׈·‡sÚÌ?Ô$/Àç‰?ֈLÍ¢s? V^NDî?´ÂI›gj–?×<Ø7ö"?Ôqo2V®&?â-Û_⓳?ÔÊJ0ЭW?±¡Ÿ/¢Þ?²8Ô]Qú%?Û«ÏbdŠ?¸¥Å>Ö?߂W&ò!	?¸Ðv–p€'?µŸô%Ò´?¢Æ¥3×?ჸŸÎx?ÆßÆÀr¸?Û¶àßØ?ƝFöGY?"ñØPâ¼?¡Æ¢ã°™.MIXED3FGL J1622.9-5004@tÛMüã¿Ñíþ`BµÝÀ7nœwškQÀ9ïÇßþù@ T¬)¿@ö¡æÅ~?ò¬œ2Ñ
¤?ïþ¼ö\í¿ÓfIyàZ¿á">‡ïø¿èªs£UNASNone?fÐØ7º±?o¯tL°?óU(6¼?ƬÄäËò?êüZ¡»é?ÆÑUý?Ql'å¤kÑ?hÉ?ƉҪ?ÚM©G4Œ?Äø³¡h×?âÐu/Eה?ÅØÀ‡*?£ 	c?»8?–®äÉ1¦…?Íú«hŠ>C?µˆ/`$?çGT›¶L?¶¬c65e?˜Ž¼'ƒZ?ã¶²?×ñ$øT\p?½è·RÖÖU?ãFñ(?m?¾Ö²~ÂÓ¥?gJ
‡šÅ?oÛ…É®a?ʀîgóž?̧$,ì-v?éHzrŒåV?ÌÄÅæPé?`'dtà?xj·žZ?ᩪp"õ?À­t'o?܋§–K?ÀãÞ¹UÃù?§ªf6²?œÖß­÷‹?ԙ畮†?µ±n•'€?ä8eÑãYy?¶úI¿‰Ô?™ƒÍ­Üíb?'ˆAÂ?ÜÀÄ3~»%?·Í⬠?àÓx¨³?¸æIÑtMIXED3FGL J1624.1-4700@u•¿ðEx?û«>ËÌÀ7öك"t—À:ƒèäö@ÏM%²—@eý€ò"@¬.õ5÷‰¿àHÅ]0¡w¿î6ý'½\l¿àY®eƒ'¿ê:"39EúUNASNone?¾jËÓá?¿ã¯IP£S?á"ÝR'î?ÐO-ùý k?Õ2*©:»,?Ïî}ù¢e=?™f½Ê'?°7££êž?àê³%åJ?ÇÛñ|Œ?ܕˆ½Ô6y?ǽ×y׏ý?Ç*=@RU?¯'wì?ÜxsÝPZ?µj0y´:É?×òm'†Ïà?´ô«îBÚ?­~†G6V?£êŠŸ•W?ß:ÜyŠ}?Ê.š"¸‡?Ý#[,?Èg°'i?¶[/ðÙR‰?·E^φJ
?ãàÛVÊ´f?Î{Æ«±Ê?Ò§}V†¹1?ΐÌZOñt?­#ÍDÙÞ4?À48@ä!?âÄ;°Ò'¬?Å ý‡TÉ?ÖÓö?Âà÷m›É?ÔmµCÝê?²±¬yù?Ú>dtsÅJ?´6`ïÙí?ÑSæG®Pœ?±ƒª!¯°»?°âd\_¢3?¡`áAMþ?æk‡s¸o¯?½Â›N-=.?Íà°"]j?º¹«Õ'܊PSR3FGL J1624.2-4041@uI&Á½¥@'x³puÀ8f­VœÀ:Â(4Òo¤?ÿØþÑ×£•@l%y6LÃ?õep•x?—{^èV¿à^]eX@Ö¿å…2ƞ¿î±Èe› "UNASNone?q¿B¤V\?k:˜Ì!þ™?ìõC ï—[?ºÛ/LZî?·9òÍKÿ†?ºœ¢ž· ú?…\Ž²q"?¢yYè?è‰×P¯?ÄéLŒ ?̂ÙՅa?ĕcn~'?¢å.–6?–4ñJñÆ?é¶*F?±Ûîx¥?Æý®
'Z}?°Q€Ðò?£HI¬ÝžJ?'ÌøŽ ?çvñààé?µr±nµ×?ÍR&´‡?´¹UÀsï?fav"Á?oÞõfo…Õ?î<›¬à??±¬ró¿4F?ªÐ4zCR?±nìŒç¡¾?'®K'ÈP? \è´
1?ézå~Ê`a?¾ŠÝ-M?ÇÞ©Û¨2?½˜Èl.Û?¦e±Ã6??™û‰dN}?é–rz=UB?­í¹I•ÓÅ?Ä墳öh?«À6Okz?¬ÿ'ðÿ?"çӉ5‰?é è婊?«µ~o¥2?č·)ŠØ?¨ÿ掺þPSR3FGL J1625.1-0021@+Âþ`Ï6@?Özúr!†À8¸@ƒ}ÎbÀ;ež8dË\@+ÐïòÝ@ô?ß n?é…ìï_§c¿ËUO
¿½­mÌaB¿äãaó Yοï¯8gOšUNASNone?h®p!¡?j{«ò2Ÿ&?ï;ބtS?¡'¿—r?•naow*[? ´è4ÊF'?p÷W ‹ƒ\?X''\Î?…GŽE?µÄ֑b6®?£å,ÄHÅ?´TÖšý?¡]¿þÒU?–ÅRĘ×Å?ëˆÁ8UB8?®Mß÷,?»@€›?«kàÌÿ§?|©2:Ó!8?y#³'^?ï¤CkY?™í!¹¶?–á+•rš?–R'4z¥?R8
D¯…?WŒÄd—…ø?ïTOà#?¡Ë1LkM?"Y}gh>?¡}RHTá?(SR¯Ç¦? áÒa\Ö?î)9.¡?¶Øg´Qþ;?©‡dÐɍ{?´¤Wž§(?£ªƒýŸ)[?˜JÕÃÜ?ëIøÏMõ?¬®=ƃ3[?»â9l!*?©þÊ}þ=?'e'v§¶š?NLñ¢¨?îкty­?"JäÕ­,?"ƒüò
â?"dœ?oPSR3FGL J1626.3-4406@u%øa¦
E@ْ]e5åÀ8®•Í\>ÅÀ:lñý2Æ?÷Q¾SEÎ@
lÞÃo¾@(qrÂÀ?à¾ñ¢šO¿îÍfØ°7¿¹4xJZm¿ïÿ¬Lh}1UNASNone
?™XÐmï†[?£€%Cû:E?¹SHlný?Àvqû‰½r?ì
Ðnþ÷~?ÂÎ.{lÖ?©!Éi'×?º~<'ð×;?ßµ:Y˜!Ê?˨|z=Î?Ý&Œ…£²;?ÊM3ˆ(ê?ÂçË>4÷Œ?©Òþîq³?Óó°sÈ?³õ ?²êÆ?áL"Ø8Þ?µÏÏמUú?ºœò-sDŠ?µçömsåš?Îåãá³±?Ê:$î:Êp?äòèÁä«*?Ë©ÆÃvˆ?¡VÇUø,?ªéqq}ø?º—vŸw2?ÀÙ£6ÃA?ë•	¤Äp?Ä;›÷í·Ô?µ¼Ÿ·?Ä1¨;u?âçí"R?Ë´MéÄ?ÔϵՏi?ÅÀ©CìÐ	?Ò:ÍH8>?°Í
XÓâ³?Óm>Â]ˆ?°…X¬lï'?ÚWóõŽ?§?´õÐý?¾ZY"a?³CSk"Ë?Ý'ói?ÄRllo?ÚêAË/?Å{¹Ø÷MIXED3FGL J1641.5-5319@tԻ¹M"Àh†
 zÀ8·Â,_Ú[À:Òð§h[?ü–$,?Ö@ªJkÞö?ÿā6÷8¿å`ý6ÞÀ¿â$¿²²ð-¿ë¥ÄD_w׿ïÿ†™v'UNASNone?Ž¶@¨Ãj?GÿMJ?ìJ«Ddö?½«Cá½Zû?¹ÓÝÉZ¦?»ÌÜz¿?‹jL
£ƒ?—ýæï9"‡?äi«%â?Ãù
t­?ÖQWUÒD†?ÃÇy4ãü-?¾žÅ	Uw?¦~ö1z?åjß4¶ô|?´EüD»?Ë ª‰DÒ?±]' ^¸P?²Ä^:B;? æiMmé_?æ]bܙ?¹dÚ®
?Ì\[W‹úl?µO7Ž¡=ß?¯
¢z¦«?±Eœ,^_?èy_ȧ?Å+Ÿ@!®&?ÆX¾6uÌ¥?°'®	ù?¡k")?¤ê0î†ò'?å+âm.<å?¾@þ•û2?ӆ
ײ?¾G2À;?Ó·JK ì?³MƸ¾?áÓ0¥K?´±wf"ÝÃ?ÄtøýXþ?¨UÛ,J±‹?À<Ä"ü{³?¤‰:† ±?æÊ,EБ?°Rрˆ?̊ÅÁ?Ñ?¦L¯‡ÌÐnPSR3FGL J1643.6-5002@tÿ÷—|À"¬_nû`À8Ì£²!OÜÀ:©>Ò£¦?û:"ˆ¹@tš{ìµu@ƒ@;ÚL¿ÐväÎKR¿æ
vrf鈿ï4·¬¡€¿ÍˆV8¤iàUNASNone?߇»›L!A?Ô&ÙÐ?ÓF±3'þ?Ï÷÷ăc^?Êc&baÁ]?ÊMÊ>¹4{?Ô¸¾ôƒ0]?ӼكÙ,Æ?¿ÎšujBò?¿ã2?á©Í7s?Ò'Î?Œa?×qÔôc"¥?·™q"†©)?Í>µ¥òK?±|ƒ™.
?ÙîÐ9¶&?ºEîn) °?ѕ¢­Ù0w?Âǧù¥Â?Ès£'?-?ȶ&ŒgF?áj€/ù?È-%Z¶
?ã;×w'€?Ó Tñk_?ÎJbçMN	?Ì|V»('?ÄÆ@´®¦z?Çc×úÂV?áw­·€‰?ÔÊ	ób§"?·NW)ß+Ý?·ÝsnN̞?×=ÇK·?ÑïUEà<Ÿ?â'$xÛ?·Wìþíò'?Ç·ýßážã?­ýHëBá?Ð
ü×Æ>Ø?³º?ƛX¬?ÜÙð¾ì?À}3O–Hà?ɗه莗?À(ËÎþˆå?ÖZøKM'È?ÀŸÇ[ÞMIXED3FGL J1645.7-2149@vay=Ùc@.D£çÑ5À9'E«Û»}À;om¿öûu?úôõj¥»;@ç²ãA®K?ðž)¶²¯¿Ç¯¾(''¿àuIó`Â¿éï¦Ä$‡Ÿ¿ï¤Ñ¦ÙÑ¡UNASNone?}JAå¤Z?‡î³S3k®?î7¯q&?µ6šÎ
nÇ?¨æLÌG§ñ?³×Àƒ®ÄÑ?—Vqð•üB?«Üo'kW?ëÜ´vi¿?Àu‡÷/ÌÌ?¾+}Ý%Š~?½wí@?®-øÒ2i?œje®Ãgí?éQ:0í!›?±#)Ž!s÷?Ã/™,ÒÏ?®ã'U"è?­'ÂË=ÁÝ?¢šJoj ?ꈧò¥?¹ŽúÒÙ&.?¼ùfñ»ð?µúEŸÕŽ?‡pˆgèӆ?"˜´¨55?ì÷;?
Ð?¿œÛz\	
?µXû ?½¼[·§?¯—½lú­š?²òSO¸mþ?ê#©'Å—?ÀF¾Ue¸?¿Õ2æ ø?ºi½üØá·?¿Ø?,÷Àý?©Ã:¡Ã]?æý×ݳ52?²ò¢y%?Ä€ò·J¸?­M@‰3Ð$?¿8Ä4ÖT?§X|¿m…?é É½—j?±>æRïa?³Àóeªä!?¨Špq_ÇPSR3FGL J1650.3-4600@u<Ãa@O¿îxd•«ÎPÀ7"`X/kþÀ9ÄÉ«?þýøKU¾Î@â¬2#?øwïzÌ¥?Ðs"k(±¿¿àÜù6¦ôæ¿åïólìõ¿ì
ŽDUNASNone?@=æ;ٓ?9|¤a
ìI?è¦14d?ÈcR¿óÿ?ÍW8ºË\N?È`ˆ|¡øI?Wò؀^?pæ
ô@RW?ÝrKÔa8!?ÁaÆÙîžY?á:áŸË?Áyâ[̦Ú?…¯×eÛe½?wâWµ]ïC?圀GtD?ºoêÒ$F?Ô€¶¦?º2PgÕ?"rpøT?1WÐqS?ÔíˆL«?º_ï{'?äíç@/^×?¼;O¸?0"¬Nv?2X5ˆv
ú?êúüg‰?ü%¼
s?Äÿú3Z?ú'C:è3?dJы֓ò?}ó#¸ë¾/?â¦m	@?ºUÀˆ¾!†?ÛЃbdh?ºÚ¡¥ñZ?‡ž+W"¥?"AM{~"?æ\»xIÜ?µ
íDwº]?҉˜Ï3S?´Ãì%†?"CÑêW?'l‰)Ú¥ñ?Ùh'ÑÖ!	?´ª]ºýù?â±Í‡T??¶ÊŠG—`MIXED3FGL J1652.8-4351@u[¼w¯d?·‹Y:À8]–
˜à6À:_yv
£W?úÎMÖL¨O@«}ůÞ?Õ	u…ÏI?ïÿî]ýG¿²§3zʯ8¿äòç
2*¿ë¡ ۆ'ÆUNASNone?‹î¬×  ®?–d–¶?áÔþ]y¾ï?Õeú×]Zµ?ÛvÝƽ?Õt ˜]Ѻ?"^fLA{?°Âí z*?×(M‹,?ʚà\‡Ñ?ãÐæÂ}O?ËÊ}1"Š?³¤ê=r"?¢pðv'Ø?áõžNxø©?·ƒ';ñ?×Tš(,;j?¶'}Fé\?´RgÃã¹?±.;³¯?ڙ†Nc:b?ÉLG#)X?à(ûˬ«?ÊAb±á†?§üËj'"?´ì°ŽÿÂ?ál–E"?ÕÑë4?ڍfãíX?Õ©Š¾ñ~?¡Ÿ|fÐï?¸˜Q}ș?Ü1JP:"?È™úßÒ?àÍc+"¤P?ɉ•ÀqÑ?Äf"É®ŠB?®ŠþœÑä?àhߝ½sF?¶Q«¹Áa?Ôû/_­ÔS?µ<Úµyß?¹Ü¿¯¿!?±b¬â¨†?Ù­0`0R?ÂVûÑêe[?ß۟²|-g?ÄÜn7b9MIXED3FGL J1653.6-0158@0ž=æœo@8ì´Zåÿ¤À8õŽŒöÀ;†"éß,@Gú~¶¿D@þ4x؄?ý'úƒ"I¤¿×'^:â˜Ö¿âFúR
‹P¿å?çx8­¿ïÊ8&¦Ì¢UNASNone?›S‹'j?—ë#&?îWñ¡¡¢?¬ %ô¸!?™®@¯B"Q?¢\ÙßTÅÇ?'ð_,mÂ?Ÿìœº¥È?íõa÷Ÿfì?º‡ˆ	¤C—?«íȽ@	R?¸¶jgÛd?¶ž«þÖG:?¤¤…£u?éÀ‰'¨xH?­ý†Ýbã?»]uÄ?¤­2‰µ¹?š%ìº8Í?Š"È]Ћ`?ìv`³¸Ão?¦˜ÏlªÇ@?µÃ3¹VS?¢í÷¯my'?"¦e[®ºY?š[©ó#»«?îñÆYE?¢>»¼)¡?ŠAŸÀäa?'h#ºÀ?}þ¤Ÿ?¡Ê–ºř?ípUcÈ?»:ñiJ'–?°]׫øy?¸,`R~"?À5×Ý÷íb?¨»Ž$à#?èë÷ÿoP4?¬íÛѾ?¸4Iß~?¡À~Ìîî{?¬¸ê*?'XÆè¹"?ìëqYd?¡Ì¾õ°A?±<¤i'Ë?˜øÈPSR3FGL J1654.3-4907@u!ÀD(NÀ°WK@pÀ9»Z´|À:Û¾	»j¥?úp¥+H-@\fA''–@×B¤•K+¿äëÌÂ:øy¿æÓ*ð6ð¿êË×qÿå¿îµN»-UNASNone	?•p.ŒŒC?ôϪŠž?ãŸÐaÏ?ÊT·õÂÌ?؏½v²R½?Ê1	"°v?Ž	äk‹$?œé¼À¼Óm?⬩8 8?ÄfÏØDû?Ù¶]½¨ö?Ä®XDZÞ?Гþ÷¹¬×?±;X4 Me?Ùå™rz)?´r0‹§Ø?Նg–DÙ?µk25ÙÂ?²‹Ø˧–"? ÅF8Ò/?ä£ á€¢?º	š"$Ã?ÒÈ
'¢|?µÞî1ëBU?£4Ert?¢ÏùjúÃ?ã(dZ…a?ÉŸâ³éÒ?×H®œ­l­?Èzuê	k?¬Ìkd8J?µˆ'¹xõ?âDPèáçw?ÀjdœPœê?×ÝÐÁµ'Ñ?ÁQáR¯i?ÜÒD–ï?³‰	%.?ÕpÛ?+d?±IX$äxÖ?ËyÀSuP˜?¬ª¡
É?¿2«½¢Q?£`ÇòƧ1?ååÊe?¯ß£Ù­h«?ÈÞ½‹?¦	pVª0ÁMIXED3FGL J1702.8-5656@tÆ]cˆe•À"}DUGZÀ8*ºŸ£ŸÀ;'8|HP?ýŒBn@K}u ¾g@ûaŽ»D9¿ßÔâJbyÈ¿å2'¤¬¼¿èSXpj²b¿é®!/>uËUNASNone?Ðñpc¬?ÂåÏ\ôø?âxªKÌê?ÉJÖGÊÄà?Ä:;ðÆüÿ?»NÆeï6ô?«§PM‹©5?³^Z2«?ãMŽv®e·?Å'q+]É?Õïù	
<K?ÄMOrüC?Ý@'s×àt?´¶¥ŽD{Û?Ö§™M)º ?´ôÉèð- ?È/¨}üÉÙ?­²Õ–$8&?Àì34?¨
q"®'?å˪ÉþÍ?¸à%#ê?ÊĞN£ëÇ?³Š@†Â?Ñ2YˆKW[?dz)i*J?ä‹Ssx%^?Ë÷›Ú«?¶ÛþAǝ#?±–s¥ÐDã?»wè]L?»7)žC?ãð吓
´?ÁCì"ç}þ?ÑZWŸÓE?¿Ä¯F?âsò‡$*?³Í_£¨1?ÒÕf$ˆ[À?±[ìì#–?À‡3ìÒ·Ú?¨ÛÑѳ*S?ЫQ›Ýî?¨ÆŸ)Y[?ãÈM?®7¦I%Cú?¿¡‹^ $?¢˜›MIXED3FGL J1727.7-2637@v}T!ÀD(@FœÒ3>À8–ØÐN,À:¶[Ëر?ýdÕ÷ú@ A]òz@k°ªØ0X¿àëïhò̀¿éýç"fh"¿ï†¾7U#?¿ïø0ðŽjUNASNone?ÍjÖ@FŸª?ÐYö:L?ãńÁÆ3?ÐîdGQñ?ø 'T?Ď8ß¼àé?œ˜e}buN?¬ûÐÂ?ä{P>—ü?Ç7ò@à×?ÖƒÿR?Ƌ'ÎÉý?ËåNù¸=?±¦";×S?Ûkª
Jh?·Îò VR@?×cK~Ùz?¹´a¤"P]? $õÜ$S}?'Ô"·õ‰¶?è^Ûö
ˆÅ?¹I«×ªc?Ê{R¯'íŽ?¶|\·"ôÃ?Á.&àС?Äå¦
Úá?èÄ.©5Ä?ÉÖŒ0¿)?·ƒà9!$?¾>éז÷ ?²‰+Ž?¶ÄíuÐ?äv{½™0Ç?Â(áð_-?Òo&9¶Á.?Àõ~ԓ·û?×i íö¾
?²ù6Nzõ/?Øýب£!Ù?µ
¶<g[?Ï1ÒÌ@5?²ÀìJ¿·~?°g³ÈÛ?˜B­Ãï?èU*Ëù£?¬­ß âM½?ÆwzïÏ&?¥Á
óOñÄPSR3FGL J1729.7-2408@P÷[ìá@AêÝYÀ8z«°óRsÀ:ÀÒ£¦bÖ?÷¦Zøt"@iÀÆY@8@üÞßHûG¿×Ù^ˬ¿ê…..€`¿ë±N¥®ö¿å·nðèNÍUNASNone?ÜLË4Ç?Ç`g–3ªõ?ÑIÍËǶ…?ÅÙ÷ºƒ–o?Ò£+çm´?ÇoçˆSº×?àKMï»Ô?ÒՔ;ᭅ?Èz­
raû?ÄûuÞϸ?Ó,ˆÝgW[?ʂç±)®$?á+И*Ñ?·(|Ihè?Ј›;ý?¨:ƒ8Î?Óà€ù~u?µÞÀ'/V«?ÃÍ°0£¥¦?¯€sSšíé?×Ú;BVM?ÃþŸÐèä?Þ>ìçkÖà?À[),°Hn?蘱
_»Ž?Ñ
ât\|?¾{òfü?¾øÆzÎ'?¼¾…›'t?·tð9o€?çŠæÛ8AÝ?Ò5»S…A?¾‡c¡ ?ÃKi±…¯¾?²ÂVô{?Üm–Rߘ?èsa1âë?®÷½"µ)#?¹—§nFï?¡µ~쑆?Á¦š§]^?§ÚIÇ{'‰?ҀhYíî?°CåÞXÊÎ?ظ3õÅ{?¶Ó'ä`Í?ÔÇd`°L—?°ykN¶$MIXED3FGL J1729.9-0859@.oõHìÙ@+&æS†ÒÀ9Bs9³õÀ;9/bÄw?úþø–T?È@
ÜTÎczÏ@må|ñî¿Øê(@§t¿ì6'üDK¿ïÿ´h¤ž?ïð¦ä/êÔUNASNone	?ØïµÎCß?ё*p}&Ø?Ù"­?Вµ¾' ?Ìn.h?Ëp"
yÌ[?+¥~?ÀRý‹?–H–þ¦çõ?±_<ÔN®?£p+»^+?µü*åã?âT;*šÕ¦?³á "Ï>?Í×l)Ai?°^ÃCZ<?Èק,gþ?­Þ͹€é?å‡F\tŽâ?ÏÖ'²!Q?·¶ ú+¶?É>"»«‰©?Ζ;ü?ÊkQ½aõ¾?ܼuË¢ïó?Òɜêd•ß?׍ùõœF?Ðlqâ_J?ÈiøtÎç?Ê`U.Ÿi?ïoŠ/ªxË?¨`BŸ‡¦D?|œ"à}¢N?™ýJq|êÃ?…Ïb¢cL?"\M?c?åyÄP–4N?³&'¤'.?ÈÒ¬=hÉÌ?­îé=ý?ÁFB€>dü?¨"ß9?í0‡Cžü?ºí›¯Q?¢th˜?¶îX žF?ªò¸m7?¯hÝÀä+üMIXED3FGL J1730.6-0357@3ͽ@gÏ@/în"ŠzÀ9Ä斢nTÀ;gæ…·?øðMÈà¯@3·«þK?ߣK¥¤¿Ú–ú©T?¶k\€š«N¿â_lµñû¿îT'BÙiUNASNone?›QÓ]˜8?³uÊ43?íôõµÏ/?Á•®LýÖ?¨wÇcÜê?ºúðÐÑØê?'L¯{Æ.?§ÑðõŒd?ìvbbJÍÚ?¿
øM?·Ì™Â¦†§?»øÖÀìnÔ?·ôØò"s@?§˜"?éµµ"ß?´É†i°?¿•y_£Î?­t®s–1?±@;8¥?ªÒ¾Í\t?ê–ù5Ë?¼ª'cáÀ"?ºä*µ?¶ðà»ò(?š2zM9sÞ?¨	º`[ú?íöÉ r?Éì%`?c?±c´>Ýø?À­<6š¤d?©â;5?Ó?±òÍÉiCz?ë
×Ý!-Í?À>2œ¹{?º¸#Xr)?ºc繯†?ÉñØÀ  ?²°`¶rD?æ¿j°ðE?¶dr&žÄ?»&S%ìΠ?¦ÖSmxD?½öbÈL5?«ó­b(ˆ?éٝÓ?´Ô"ž'.?³¥3í?ª°ˆ@ÓE<PSR3FGL J1734.7-2930@vd*Ã") ?û6«Þ?»ØÀ8•—Œy§À:zŠÊɽN?ù¼Á"Šf @¡œò¿?ö>À?°uñWrb¿åýu·¿ç$ù³yƒh¿å¶$ÿ‹2pUNASNone?Î(Ž츥?˳_Lo?™"X%3?£¥Ê€F€P?ç¬É¼n}.?Í(gk²Å?ÓýV ~BÚ?Ôß|uO?ºp"ì'ä?¶Ç­J\?â¾f«cN7?Ó¶—½\©?Ôø€ÝéˆM?µt"4þí?ÄИÈ»ú?©Þ'°¼ãÛ?àO™‰œ|?¶ï¦‰1»'?Òfý˜'Ô?À¡YiÜEC?¾î•I}Í`?´ËUïÄË?âïØê?Â|Ô@MfÕ?ÜÞŒ,"?Ѩ4­íʯ?±Ê<^G?¸‹‰´¿Ó?Þ¯aîmŒ?Ñ¢•j¤¨Z?ákjÎTó?×#mâuo]?¹q¶D?âþ?¹g«)B?Ö̼ÒêÚ:?ÓP`µÍVà?àHÂi>?¶"nP»ed?ÈsŠû­?©"Ôѽ?Õ«ˆµ×Îð?µw9"ò"~?د ]²Q?¼ÀD,™Ý?ʑù V¦o?²_‰ŸÈÕ?Úã5;÷?¼fy—׳ÂMIXED3FGL J1736.0-2701?àWà[õÊ@iÏ!:ã+À8¼°³ ¬À:œ÷½;_R?ù®WÙÛ©	@
1î¯ËŠ-?ùmª*5ˆ£?åËñ»C¸g¿ç¼—šˆNe¿åuµ}"š¿ïÿáïôšUNASNone?—?UÁ­¨Ó? @8WÉæJ?À™/5œÊ?Ĺ9¶ÉÄô?ë¹"צ×?ÆO‡Sé-£?rV‡žzç?"WØð'…?äyü|#"U?Ä-uÄ}Gÿ?Ö¬êёû?Ä?9_áÖ¹?Áf-0¿Ñ?ª¼°*¡?ؽ"†Æim?¶»‹'âõ?ޏTàñ¶«?º}'Ieœ? "Ù¥/?'Zëî?â`žÀ
æ?¿Ðs<=?ÙÔüÝP?Àªs†Šs?¥7"±(?­UüªÃµ?É^;"=î?Éâ÷"lPX?èTÿÀâUB?ÌAŽòÿ4?‰³´'±\ž?"L'M`?æmœ‹;‡ë?¼îù{	>K?ÒW)DûeD?½«âÖ=S?ÐxÈÜ°Î?°xùná©?Ùj߇dÉ?±ã>]›­?ÖWš×Ã\?³"ü…=?¨ÛNÙŽ›?—•¹ÌP6_?ä.Ý&ûÜ?´ÿjýc"Y?ԆÛáè'Ñ?´Ü`õîlMIXED3FGL J1736.5-2839@vr÷eýŠÛ?ýn'«?´KÀ8—cW¾,÷À:´²G^?þqõ0K¦@/° ?ò`àëgÿã˜YþyC¿ÛΆXÒ²¿ïÿñÉ 6[?ïöúNKx¶UNASNone?ÙHí€\Âà?ÓñÒ¤Áښ?Ñ61?hÏ?ÏQëò¤D:?ՀáAMþ?Ò1
S¥™'?âë2'M?Ø^ª5Ú=µ?¡k´?§žl¯?Ù¢É7Y^?Öõm±çÍ?ÕõO
•{
?²âî|héö?ÓԬ֞mû?²ª¹ŠL`?Ö6Ìø?´uÐK¦Te?èYç+ëË?Ë&fhŒ'ã?žL(S"'?¶TãٚÞ?ÊÎÞE¬BÐ?Éæ
‰N{l?Ô¿¯ 2Ä?Ñ¥äÚÏ]»?Ӕv÷z—Ã?Ðç^éÅ?׫Ùèi5y?ÓAŠ(Ґ?é~Iá9Z.?Ói‰íLû?•Ý\jx¿? j]–+?ÇK,í&'?Ѳ"³8?×ñ½Qړ4?´#þè^ëÌ?ւ¥!ô,É?²rûÂ
)?ы‹_D?²|àƒ~sO?í'ÖŽcýÎ?´¿/Ü4Ën?‰s¦ò›ß?¢Ùr:@ù?°:Ö®ú‰1?² ÅNQ'\MIXED3FGL J1737.9-2511@B¡µÇ͊@~HÀc1þÀ8O#—´½À:ÙXÌIð?ý
Ä<°`@ªNò]U@ÔäÁ5>ü¿áð²Q˜Æ¿é8¢=­	¹¿ì5Ì>ïÿ>"Ó—uUNASNone?Å-˜G<³?¼ìÕo¢i?×çٚ³?Îû4åÌh?ݵRŒÆô?Îɽ)Qï?­ W?´ô'>èY?á3"µÿÖº?Ç
ºwN"â?ÙæÕ¯ýçª?Ǹ•!(³?Ï(ãÉ\?±çêƒ*½$?ÖŲ§1³?·ˆÉ@§ð1?Ún¥ÛØiŸ?¸KOF<¹ê?«ý˜íXOÑ?›Wvt֊ž?âÏ-ì''?»Dtº³M?Öáñ	 ›I?¹fÍh5ðé?ÎñÞ:n¢?ÆIÌ8
Ÿ?Û¯—¡¬?Ðî۝þŒ?Ô×yß"!?̈ëM¸¼í?ÀˆïA/¹ñ?½ÖÁ¶K߅?á±þ³àÓÑ?Â%‰£¥Z?ÔWŠ÷¦{f?Áù<0K¼?ÚÜs¯á@?´xÞ×ôð™?ÓPžF/Aë?³]ϊ‰‰Á?ÑÓGF ÜÖ?³ÈìäŠ?¶ÍåM7›l?¡†M]<,g?äÀƒé.,?¯ãjù1'?ÒA¤ÕÍ?«Å°Í-iMIXED3FGL J1740.5-2843@vy>Õ(?ñVWûi˜À7kŽ#CÑçÀ9Ó=¶CôL?ùIA<‹@³¼Òì™@ir©´¿Ï…Xþ㏠¿ç»³Ï½¼¿é|ç´Q"T¿ènÜ*ÝUNASNone?[¾Q¹KÊ?aiÅmìB?°c/ø¿?´•YÅÊù?íåºØ6@?´Çu›ž½¬?˜½•)ûڊ?ª®Ì2}h§?Ö×VÄQ?Å¥òå³?ãÎhL‰_T?ŧÅ°?´Þ«"am?£w‡7ÈÍ?Ë`
K´?²˜‡nJ–?æŒ'U¯^þ?´·UOqb?–|¡ú۟?'uüÕÙ?Ïh–¬Õ5§?µž®ØMÆ?çqõEj)?·Oý­Ÿž?U!½o'³ë?Xޘˆ–Í?·üÚÉD?¿àÛL—]T?ìõëæ(ϓ?¿þzªý*t?¹+PAµ"?Ãś€£Ô?Ù­g²çH?ÄQö¨úq?à&¼ú"(?ÄëCããx?¹Ø%|ƒ?¤¾zÕø?Τjù7É?°é%§g4-?å5J=w?²Ì';|Y¢?œzF‰?˜#‡$¿*Œ?Ñ@?ŠiŒ?°`'‹|L6?懗&?´1¾òå'qOTHER3FGL J1740.5-2726?妟ê$Ì?û»èÿ2z§À7ù/‡­À:3µ«HÇ?ý§7è¥@1	½@ÛçF÷¿Ùv.ü¨î²¿è{+½ÑÞ¿ê'ôRLÔ¿ïÿ›o÷M™UNASNone?†¾+"'?Ž¨!§§™?ρn¬¨a€?Îw'Á~\?çĬSÞ?λþÝm7?fáõû?n€
B?å7qž}Ùõ?Âyφ²Ù~?ÕcY¾Y¹Ò?'邡@¾?­.MÓïí?Ÿ·
x§?ÔâŒs@i?¹† ¹•ß?ã¼
ÜPg:?»Õ)Ÿƒ
?Œƒ/†1'?'Œ´]Z8?ã; 8Écû?»-i¼ÿq²?Ø¥¦C}?»|-|SÒT?nM1ò"£?zUŸf† "?ÎSÎøåÉ?Í'f¾?è]ÚÆàz?ÍJìÿ6?}_øÌü¾?‡8œ˜k`?çíJa3?¹51­Üs?р¥üBJ?¹ÌaBD?º(i«V}?¦Ök¼N•Þ?×;r°)[¢?¶ÓP¤9.?á9†Uç`?ºc·Åy?"ÅàÒñ²"?‰$,¤
?äTÀ`¸\?±T[aèŒÎ?Ö!2™t?±þüÏ!CMIXED3FGL J1740.5-2642?ôÞ i—sO@û¿¼CÎÀ8ÏËRyI˜À:µ½Ñb^?øºQO}ì•@ìG'd?ô4đ?¿±ïGºU†,¿àìi9i¿æIæ¯æ¦×¿ïe­¾ê‹úUNASNone?xÍvs*?}X¤Cݪ?æO/)ۓ?ÏtCÔk&À?Òÿ+¤s'I?ÏeIG"
±?e€E-.Rù?yEá4Œq?å—"@7ã?Ãçž8©ƒ‹?Ô¦ºöáÄ?ÃòóG_åï?®K8;?›‡F–ùg?äéõ"ñ
‰?µðlÑ~r?ÒiLS"{>?´¯77¨!˜?œbr¥‰ÈÞ?''ÌÛÅ¡?å6ü{'ð?ÀÚÑc=?ÓËßßE—±?À"á#
?€ˆ³vL&?†Ð¬,"° ?ä!½@#í?Ñ»JÌà?×8EQÿã6?Ñ
?O‰˜?"iC	"?ŒÔ Jš¥U?æÑwù%4?¼Ø¹™X?ѹÅ[ò͛?½K{Ç8£?ÃKZ'›ô=?©+KfU?◩§%?Í?³çl«çß?Ñ*ÿhç†H?±q?¦ÆØ(À^?–ê›°CUõ?åÎg"cϳ?¶K4*ÛÊ?ъUՅ¿-?¶Ëý>x™kPSR3FGL J1742.6-3321@v>p†nD¿üdóºw_³À8)+hc–¨À:wfÀ(yœ@kä'fI‹@˜?&†}?öñ ԋÝï?ËÄÇ>\Jó¿á†ÿI\ül¿êôϺÜ¿íô[L
lUNASNone?Pa´hc?S¼ª¹$?û?ëÑj'YR?Ãh,S	I?À™4ôXP?ÃbÃR¿Ya?E^¾‡5°?e'bÏ7Ë?匚ó`à@?À<b*=c?ÔܺÒ]?À:Žpú?–Â?	U-?&DTœ#2?æ9–$LÄ?µøŒöÌdB?Ò ¯ÅLrA?µ\T‹§Ñ[?‹¼g,'¿?'aôhÔt?çP©)$ß?¹¥æ0Ãd?ЀɦI!Ô?¹oÓ
ãÖD?Aj¿µZ(?Gə`öW?í£Öa +o?»Ônv?²¾wv8~g?»Èäà¿ÈØ?XxBl?¼?nÀӕ??æ{'|ònó?·öÊVÓL?Òð'ÃÛ?¸[eL"'?¡ÐBS1Œ?–€k>J:?ç:RLå5?²DÏD6ÀÐ?΢´úŒèJ?±Ú¹Ò!µ?–JTM?‡^Uì]Æ6?ç‡7§a-l?±šÊ¤²?ÏÃq?™"?±9Üß_9PSR3FGL J1744.1-7619@sѬ<žìÀÀ6x›ÇqC9À8"{?;2À;]"mé§@W±\®×™@'p\"y?ó¼†=Ç5ß?të¸cËäÀ¿Ù&t;™½¿åÉâܦ'¿ïÿíkÜOªUNASNone?‹'ðLUY?•T™a®?춿s>	?Á Uí¿­ø?¶×ãH$·?À>Œ^-îâ?t¾R"[í°?£÷ݕɊ¶?ìö´ç¾Í?ºu&¡ïi?¶þs¡@	¹?¸2žŒ€S
?ŸÅ=rw^?''X+Ú?êºìMx.?±(¿*¼†?Á§Óež?¯Ü8‹Èܹ?'¸Leäc?†cF?b="?í~|Þ´%?§MŸ™6?¯<âËâx?¤Ä£bº:?ƒV7Az;¸?Ž˜^ ÀÁ†?ì¿Ýbi?» ŸÈ1Ý?½/@³pÁ?Â4"ÔJ‰?€Î7â?ˆŸFˤ*X?ìÐA7œ"8?·ö+›ÞD#?·zdžÈÕ?¶‰q'Ôh?¨ÊB{G‹?›¸™žô?ê]";ƒ?¯z¥ão?ÀXæùL?¬Æ7f±€?¤?€û;jÒ?Ži mao?í8¯-­k? ˆüMÏÞÓ?¨5ð1ð'?š'ÄapÉPSR3FGL J1744.7-2252@N8C=lr@
©‹XߕÀ8¢Á¾{Ñ2À:Ò('fvW?ý 'b"s@^ߥ—~·@÷§üÞ¸]?¸Ø>Óp¿ìZV1ò¿çRg!]ƒû¿ïÿ'Õ/FêUNASNone?²1‡äØ_?­Á3³Ù]?â+N;2—=?Ðã‹U38?×'Ní?ÏD¬Ú`€–?ƒÍþ5Z–Ù?"âò†£?ãm9æøêY?Ðï͔>?؇@ŸÏ¶?Ãß
9óIl?Åö'ÐÉþß?®%×pÞZ?Üd—·Ë?·¬d¹ÄÜ?Ù73HÆ?¼
|™dC?ªŠdó¹d?"ˆsÓ?å²FôÊÜ?·C­zˆB•?ÑJ©Ewó?´»û}Á:?±æt¥A¹ ?³ªe —?äåéÙ°?΅n5à-?ѼA«[8?Ícy›ˆ˜?—ÀÀC	fœ? wW'"?åŠeî‹'U?¾S^ï"¾?Óo('Œ?¾ÌÑ:«Þ§?Ðìµ!¬Åh?°ö𷸓…?ÜHt‡€+M?´SÞ±¶!ä?ÒÊÖVÓK?¶¾*Zûð?¶v]øM?š
lš¾û?ç²çó?¬ÛÚ6æȬ?ÅüÅböw?¤˜ Pf ¦PSR3FGL J1745.3-2903c@v}Ò½<6¿"" 
êÀ60•âTôÀ8¥ãÛÝ@%{‡ŠÎP@	ùù€´ñ?ô¡9óÁ®?æÚcY\ë¿à'î}î垿ç–Ûñz¿ìk]ãyÑAUNASNonep?­¸­hò?uþSå?âG½éÚú?Ôwéä"E ?ÛnùQ)E?Ôx[o΀?-ò›ÁôÆ ?dii›Eß?çêõÀ´?Á‰HsaKŸ?ÐtëÁÑéd?Á‰ØnÊÁ?iN´°V¸‰?fsïŒ"Œ??èp,ÐîoŠ?µÛ¢Aå¦Ù?ÍÚèÏ{˜?µÜ-ŸT×c?Bº±uŊ?M'êô,ä?Öd(zæ?Å[ôÓ&-;?äÉ=I¾þ?Åj°ÅQ¥±>ý¸—ÖD ?£%Ýí²C?ä¼^JFS?Ómû)Æ;Ó?ֆÌâ5-£?Ón¯qa?BÂ5'|}?d›Ø8:Ùñ?éžDÏöx?³a-Çl?Ét*ŽâU?³jÀ""BÕ?lõsEH?wÐ>Ò9Òk?èãb/Aƒz?²_Úv§¨Û?Ëþ¡wÎ?²L°–l?3ý/jBã{?H`½c l@?Ö8¥Â‹š?Áë4xÏìß?äá-xÍàã?Áù.†ƒ}MIXED3FGL J1747.0-2828?áÔG '¨;¿¥(ÚûÊÍTÀ6¦¤Gr…YÀ9Æé]ý@úÁC`Ó@ÂÁ†º?ûtS5G¿Ä34	òÈ	¿äÅHEWç·¿è]xãQÛ¿î"ËÝUNASNoneP?wCè>m¦?x‹¢_	֑?Ë厤Àa?ÉË^Ëðâ^?èØ3´ØÔ?ÉðXëÝð?_Ǩ²™v?zµ¤Ì²Þ?ßۚ2Ï=É?ÄgÜ!l?àOd†N?Ä;Ž?¦C 0	"¸?ŸuT'K?ÚË+U?º®þŸqŽ§?á6?ç‡÷?ºáöÚß¾?‹-ê(e??‡
ÊxF©+?Ù±>fmc?ÁÂò-"s?âºèJ‰?Á@FExsô?"¨×R'Õ?+ü'h?Êp7«=?ÉëRžÞR?éN¸ä|[?Ê:ClU,œ?n{ìÝPå?ƒóŽlq?äÝí[š]?¼~²•?Ö-n«·Ý?¼­PÆ$Z?¨S:'1¢8? dà˜EV'?Þp/ à'?¶¥Øµ@ò—?ޅi
,/Ö?¶ßåÜ9è‰?‡ÙÙÔ³?…ÈÆÑâÀ'?à<ôjÔî?¹Ý膚A?ÞÎaՐž?¹¤ó²ó:}MIXED3FGL J1748.3-2815c?ìà³3ž"¿Å#rö"À7âÃ2ðUÀ:h)qéQh?ÿ'´µÔ¸©@9›
²ái¿þÞ²G»U?åiáypô?ƒ4K´ýÙп͝D¬q&¿ê"ªúƒÙUNASNone$?ÅÞÁ5?ÓgmhqÈ?æ§ä­ê?Ô3$͜è?¿´…-Pñ?Âé;ĸg?É‹™?ªîèv8¦?㝯Z›?ÒO8wjÆ?Ø6´H,Ъ?Ñçý3‹·s?«âií£ù? xˆÃV®?â׉ŽßZ?ºõzÍÈí'?Öԟ¤ ˆÌ?º<
µ±c?£ë¹ïFì›?±{ÒÔx½¬?كAq"?Ó:ýO²¬?áÿ£¨€/?ÓÐüD½&ð?Á˜$ØA?Ð3úusìÙ?è	ákH'?ӊP­0i?½{Ä\öB?Ä©8;8mã?•:TJì±?¹Úïݏü?æXï9øä?Ê'mؼ3?Ñü2ÜÝL]?ÈÒñtL7?ºpZ›ü?§"ûY¿?á΁¯åWÕ?¸"<}Ð?ÕÆåùTÑO?·ë¹d¿\?–(l˜ ? ,ueóÿá?ß¾|5
['?џ'hòÕ?ÞÞý"Æ?ÒA¬ŽMIXED3FGL J1749.2-2911?ȦÃ"Ôì+¿êתv`¯À7Í«û›í1À9®"ñ¹ì?þÐâ»Ìtb@
ۼܿ´?õ$ýÍð
?ïíßvȉF¿Üن±+þÙ¿çLÞ±ëcÖ¿êÅùé‡åßUNASNoneD?+ržÔD?7¡Þ¤69?á"ÀØ?чMø…1?ÜôT+·z?чg½Ôal?KËhÒA£?fe4vÏ÷?ßÃÁŒ÷?Ä(Fì´¯Ü?à,¶†(<?Ä3!;J?%?‰igyk8Ï?€Õ¤,XZ?ãz؈d4?»TNL¥[?Ø?´H$:?»Õ0&A?ýe®Ú?'#6»Ç?Öҁø==ù?Â
wjxLv?äNʞ§Óø?ÂsC8äÍõ?þH…d¾N?ƒÈƒ;¤?䵩ùß?Ñø¡§Z!Š?×ñ̹µ '?Ñø¥*ðj?WmÎ
a`ò?v³åN¾žö?â¢c:Éå?À,V`c?ڣ˼{?ÀK4íٝý?""Ç,6Û-?H§-J?â؋+_?·kC-z‰?ٝ6ÃFÍ?¶èŸ‰o@Z?þË?ã?…xöb§§ë?×ÿeÄ]›?ºÞÒÉ;â?ã»é"¡s5?¼¾¹lPiMIXED3FGL J1749.6-3133@vcpâÁ*ØÀ×)9µ-tÀ8²²eByøÀ:u'OÐ!ì?úHDºšH@
ÒòÖ¡¸?û|½›+•¿ßäk•ádp¿æîrÇÑC¿æŸPµ¥ô¿ïÿƓðÖUNASNone?ƃø—ÑQ?Â4í+«Ä-?¸rÄ Ìkc?¾‡+™P?çP©V-¼¯?Ȍ%vËÓ?¯Ý¥"Òõ?¹×CïÕ ¿?ÕßÚ׸Ÿ?Å&¥ú-¶¥?ãr5¹95ð?Ç­Ûþ8é?Ѐø¨Ã?±"™tI˜?Ó«Û-Á6õ?²d+³?ÛÔ"ٖ+G?´²Fà¸\À?Èã
ˆ¼t?¹Kœø©?ÐA¨0¶+?¼üÙ·–Û?á¦\
AøH?Áï*¥p‹?×Òȍ*¨ÿ?Îy,ãI!B?½n{2Ñ8—?À¹"­?àhÌR‡?Ïb*A[?¿GöL½j?ÃÈ[ãF%?×þ T¼Î[?Áæ½Ar?àñø%?Ä¿.zM	Y?ÜÏèØhƒÄ?µ¬ïeª´?ЁO8ªôé?¯mûí2D?Ò®Çïÿh?²Š:M{*e?Íü&à=?·ñv¥MØ?Ù¹ôœ¹N?¶»Øæd??×é2›U'ò?¸€¦,\ÑÓMIXED3FGL J1753.6-4447@u±]ÌcñAÀ"Õ5†Ê‰üÀ9dßý+9jÀ;cìƒKy?öPrß­*@
·²ˆÓÏ?÷Y˜1å€M¿Ùl°f:¿Û¹Š¹	ª¿äT*\¨€¿î·(ðmUNASNone?‰Ë¡-֊¸?‹î>v-9ç?êŠ^ÿG|?Ã뺒|?Ä:àpî¥?ÂÍòÍΐ­?£qÔrwZ™?©+½Ž¸Î?äé
dKÈÅ?Å	]lԃ?Ó¿°©ƒ#?Ä ¢6÷
?Ä"s4!'?®®-'¹ð?å@Bêã—?¶1=o	>?Æ܄¬2ߌ?®¨O¬·?ÇÑ5ÖëN?«aˆ×ö–?㣀S³—ƒ?·†Áùº5?ÊU-{Z¶§?²â'à.N?/«™jW‰?'"bè€Ó?ë¡|É̉¨?À.–R?¾è.ΰ¸Ö?À÷ꡍÉ?¾QŸô–Y7?º¿äuÏ©»?ã²Û>¡ô?Á嗒
ƒ?Ñ–Mp‰?¿öVbQÂ?ÖV1ØÙå?²P®Ñs¬s?àk## ?²'Š°v¨?Á§M
œB8?¦Ê؏zf6?Ô³C ?¬yoÕm?áʊɃRl?°˜ò뇇z?¾ßI|á?¤¬ÛŒJPSR3FGL J1754.0-2930?ÜÖ¦ YŸ¿ýÊÌ&´Ÿ¯À7çå7&ݺÀ:2ËÏvË8?þ_¿c×ñ@[çÿ@G$êp Ï¿áÎ*2-¤©¿æ¸€"åÕ²¿ëÁþ¸,VË¿ïü»8¿}ôUNASNone?qaFBaÕÚ?qÖ?ÜU/?àzßð?Ðؕ}€3l?ߺ<®Ô`·?ÐÏ0"÷?¬?h"âlõ‹X?~ÑÝûlÌ?ãD1ïÖ?ÃÒ,#/Á?ÙFr[£P
?ÃÜgÈCÙ§?µq~Ðôx?¢÷<$-Ò?ÙTŠñ¶?ºG4ïÿ_?àÆ¥àh¤É?»ûPüع?žÐ<Ž"»?'ËEš0EØ?á²Ð«îI¹?½¬ØÙ©Ó?Ú­Zߨ$T?½—Vôk!?eÛÆ|‰
?pyÎÇԍ‡?â¢VgHl3?ÑsPçp‰w?ڏ›¤
á°?Ñi0ÏÅip?uˬš<?"ut›VŠ?ä€Kÿ?ºëªüv[?Ö«:—fÊ¡?»')¯?Àn3‹?©"ìGÒ¬ª?ÛìûbÙ¶b?·cÌK¾1Ž?ÛÛêפÂ?¸"/Þo*"?¤ÏðõtV?—3Ö8‰Èç?ãj|úÁ@–?²åg+?֑ë—úC?²eÉ_ÒEMIXED3FGL J1754.0-2538@?§ëkôE?µ»Ä¼²ù<À7æyó$÷À:T9ܚ *@wp×ÙpI@ÏôTüÊ?æގ¿‡%4?ïÿ¸$B`¿ÑRôþˆöM¿âaåí"¿ë#‹²(›UNASNone?±‹èæÈ?¼^è©ÞG?èézh¸?ϋ.Ì
?Ç(""%2®?ËFW_.Ü?g!µyÂð?‹ˆI©ÛõÎ?Ü^/؂/?ÉM\\ÕÍ?á¹Æ^.ð•?ÉT©+BÓ?¥ð@"H;?œz¯)Àò
?ãv(‹ ™?»¥àò((?ÖU¹ÆñÒ§?¹ßÈýà@?¦..}6?Ÿ¹­s0È?ßëa*H?ÄTP=žàÅ?ÝO$ÝÒP?ωƒ"x?Ÿä㺒)?°þ-"J?ëNÊí"Zª?ÉM›ÐfÆo?½o¤R°&?ÆMpÝ:?~íðuSØ/? ¬SQ(0?âÛ¥œv?ñà?ùÈ·?ÛtóO9ñ?Ã÷9,W³?­]ŒˆpÅ? ÙŽëÚrì?âŽ\|$?¸
®¦¦Zc?×7–=ÞK¿?·tHWÕ?«EúהTu? :»t½?áÇO82³?¾L^õ¦,F?Ù	",?¿lÄÆ»]MIXED3FGL J1757.7-6030@tÐ,<žìÀÀ1*$š<À:W"'iÑUÀ<;¶N?÷6&:&l{@{QZÀè¿óñF×Tæ?jiЬ<øÇ?ßÏ|k¾¿Ï	K®)I¿ë¹KÕZSÍUNASNone?囒Êk2?Ô=ðŔ8 ?ҚNnç®?ÒòGjÍ©A?¡t_åx'J?¯Éo)èä?È+ƒ'g4(?ÎøK'ßø	?㱆wuNÙ?Ò!{F-?ÉbŸÃt?IJ"&›u<?Ö¹F÷Ïõ?¸vÅf‹&?àüïJ·DŒ?¹UÚ^)?ÀÐG3Mé?¦îÎéØWb?ãJDg–š¿?Ïó®ÔÐb•?ґa±ö²¤?Í¡>"l?»hUûp_u?Áv8Fÿ
?涱¤Êœ"?Óîð¬-£…?ЖÍÕ?Ò¦"ï?¥?Ÿ¼û$wNX?¯"	Éó?Øä\°?Ó£cÐg"—?ÝÒ)}§ËŒ?ÓN²+GÉ?"rãø7Š?¼k­/N?ßÔ]Aqô?¶…"Tëp¥?ÚÏÕ?âîø?µšŸeŽä°?µo5ùÔEQ?¡Æ.ÀÇ?æõQö¿ƒ?ÄæÝ&-³?ÎÀ«Mm?Ã>|J‡?¥¨2'é?¯°?'´Á6MIXED3FGL J1800.8-2402@ÓW>«6z¿ÜíWœI!\À7VIÿ''ìÀ9¶0©ë÷?ûepÈ@½ÉljÁà?ù1%'¿Ò
'ús¿ãÈÓÉ@PR¿á_)oÁë¿èᏄ—ÔÈUNASNone?W'Í ðë"?Y"Ëçá"w?ªq"ˆ­'ˆ?²˜ªa1?îM&Q"‡i?²Í[X!qm?eñÐ3&ý?{¬—@™,?Ԇ Ëž×?ÁÊl‹¢?妽ÉϗW?ÂC"~?¢FNéƒë?"¯µÿo¦?Dziõ:?±²>
'??éî"¬Ó?²á¨Y@‡0?œíæ{^?™˜Ô…zi-?ùRÚËñŽ?³àp?±…n?ê1~ÉùL¡?·ìnA•æK?RÃíGÇ
?Y¡Ñ¡o?±"â‡(?·Èb÷‡e®?íÒAÆoö?·õl/"r\?u«­|¾*?Š^T	œªÔ?ÛÌÃ;˜KU?À/g\ì¦B?áîHP·äš?Àâ+ óž%?¯AÂqmð7?ŸV®±…~?̓dDçÕV?°Cwˆ~'?æç
Çjsx?±áxmR?š˜PM³,·?vâËÁÓØ?Ïûu¬ªm|?³Z"ÉpØÍ?ç,`0Ñ{?¸2zWTPOTHER3FGL J1808.3-3357@v`÷<ÉÀÚ\¢˜EÝÀ9w;ØbçÀ;DŸqIï7?ø
.j€@oÅz¤6?ôž9ŒÈZ¿Ö¾l$žù^¿Û‹ÿÅ*¿çVïó9ëV¿î°¸ë!)NUNASNone?¦¨pœ×.?§6k`œ?ꨛí±É¼?Âû'RRˆ8?¿ºÌYµS	?Á1–a<B?·Tû͆Õ?¼	T´ÚŠ?àÀëƒ#éó?Æõ=N#F?بê:ùó?ÅàäNýÓ?ÃU‡H*³?°œ³àò½…?å>mM'·!?¶êYY×p?ǰÁÊoû?°ÁVv)3?σóc˓?¶]@\?àÊ0?/b;?¿ñÜaüZ•?ÍS¯Þ«ƒ?ºI]'^¤â?­罶Q?­Z7H܏?ê´È£ê¢Ã?ÂíIöTkÎ?»Ñ¸j¦MB?À
¬$ûPÞ?Í 3ð%'?ÉP.8w?ÞMv¿¾¶#?Æ_Lƒ]ºh?ÒâoH.ºJ?Á±ø"¥Z‡?Óóu×âCp?±s:Ĩå?àÿv§@)?²ŠåéOü?Ä9µ`ýú?«í7wüÀú?ØwyÒ1™3?´Q§;¾~?߆q>Ê?µ9½Ãã¦?À)ߑ9h?ªàÞ?w…PSR3FGL J1813.6-1148@2OµIùH@³Œ|z¤âÀ7ÁÐ\¤EÅÀ:¾­OY?ÿ"VÔxß@¤[©ôۊ@¸½ÄMc¿ÝˆZá'Ĩ¿í7úb˜b¿å
V<-E¿ïÿYƒ÷=[UNASNone	?káµ¹ù?ueÑëÂ?ÖՏx`"?Ñ#̸ÕÊ?äyVÖAì?Ñ%a$tQ?T]dŽ\ë?nžñ¬±ø?é!Ì}
††?¿#n¾¦n?ËP	Í3O?¿$°ÂÕj?µ!9Hÿ€Ý?¢'0¡`÷â?۝4þ÷?¶¿äB³y'?ß yKŠ1?¶Èt½0ƒ?um>Ré4v?sØU»0?äåBÕ+…?Å5©É×=Ù?Õà€Ó
e?Å$!£Ïä•?C'"cÇÍT?Nä¿Ø~Æ?Õ𮵭?ÐÉ`‡C?åÈh¨Ï±?ÐÌ)]`G,?rZBÝpl?'ƒÁíªû²?éóÞ\þCù?·ž.Ѩ~?ǟ£ºÀìÖ?¶à(¿ÔÑ/?¿ïŠ§c[Å?¨ý9ø°f¡?ܾ§5¶E?µx¢‰‰?ÛEv=Sˆ?µÑF'nXÌ?wќ«¡øÆ?r‡³ô©× ?ç¢]yœ'â?¹ì¢ÚÈl?Ð[þ›t§?¹übÛ[JMIXED3FGL J1823.2-1339@1š¥ç…µ·¿¸€,5=$À7jf¦'GÀ9R[Æ?ùJšèùÿ
@䓳%±À?ýwã:"¿Ø`ð"¶—¿à¿Ÿ×eü¿ä5†‡8¿è"†¸ýsDUNASNone?l/E?]¹ž?l™TÀÊ?Á:¶±¾?Áèà¡vþ?ë•KM1b?Â:‰ò:M?a·ÐV90š?uINC(Ž?ÔPûrI?Á`aZŸ?åÅÊvJ"þ?ÁŸ 'xûû?¥ë¢tæZ2?•g8"j¾?ŹÂR2Ò?±,Ô+Ë;Ñ?é2ÕD7ø?²¨cfû¹T?"j¢Â)‰%?"¶piõg ?ÅîÜvãâ?°œÁ›óv?éàóÌQ8?´"§øfŠ?bÛÏMø]?nĕ|ƨ…?¿ð·føÌI?ÃӍT֊Õ?ëïÙ7¥nö?ĆfOÚ?rÏíÿù?"šxtν?Û2—×͇?À€paÖ£?âQÆÙîžY?Áãr"(Á?³kú1p¥?¡ºvlš'P?ÊãöÈ2?°c¥ëÝ?S?æك:ÌH‡?²Y°	°st?"çp€àT?™/‰·L¨'?Êjñnuð?¯ c¬/šä?èÆ qä?´žÑD[þOTHER3FGL J1827.3-1446@1ud0+A¿÷½¢!þW‰À8ˆÿI ÛÀ:•ýʛš%?ö'Ò€@
'Ü®—,­¿ía'ÞÒo	?çtÝ̃¿Ï(œA8ž¿ßH–3€¿í³rB_ŠUNASNone?Âðû¾@²?Ðö*'ú5?Ûaº›?Ò–Ï~œ­?Û&9t.¿Ë?ÐÚÅSm?¦yPù¤?¯©V>ê»?ßpW¿7@'?Ñ`+3Šq?߅@¬B"£?Ñ|^k¬\¦?¶/ï•
hª?¢`J6ë?ߞP¼Êºé?·7pöß±?ÚÕ³^DaŒ?·<™Ò8Aq?³¯ÒHÀA?¸0åɲ‹å?Õ¤@À?Ї&[D°o?âÊ¿yR&h?ÑÇãáÞ¤?ÊP¨¨Äô€?Ñ<,¨Ìߺ?×яp1&¥?ÒÍ3cs†¤?Û;l_?Ñ3²_½]?¢õ•6:é?½;Ò¾ÿ/?á‹x‹¤Zà?̗Y\z?ڊ\Ak҃?Í
epi–ê?ÊÓ®ö™¦?®¯Ñ¢4?Þò…ζ†å?´eŸD%	T?Ó£¢¶<¬H?´vºÇÔ¤ä?³?¯‰V;²?³u-*dëX?Öµ±Hž±?Ëûi¥,—/?â=1jÊèá?ύؐzaMIXED3FGL J1831.6-6503@tŸ?¼À6gø"»ì«À:‹†³
&À<e»À5Ö?øð+oð@"˜ýgtX¿õÇlãË¿å뒙0yV?Á•î¿:èß¿à8ƒÝ£<¿í…̘IhUNASNone?ãµ<­…^Ï?Ö}½.Á?×䊍Pú³?Ö0Pª½Xf?†'Ü{±ö?"/+N¨Ó ?¹Û/n¶¾?Çm¡`Ÿ?ç\M"†°?ÏõµAspn?Å¡1úŠ0?Ø) h?Ñÿs˜~§?´E¨šH?á	zÌ
@\?¶{ç·FÄ.?ÇÛ-žÚÝB?±:.þH¯?ØCÔy)4?ÐkQÃ$?ßÀJã©K?ÑOõDÔà?¿ï'Œë>?ÅôJ•$"à?àãrŒ±Ì?×Ò|hu#1?Ýf¼¼M<Ž?ׯ¦õÈ]?ŠfKçÉ£.?–‹p0~H?ԁ'è̘?Ó¦CR²vØ?áG1T`Õ?Óý—è6;?Áàwj€ã{?¼œ;VåŒY?Ù褵'¯¬?·»Üú`?ޘHê2@ø?¶¤\Ÿïó?½üI€ì=o?§°Ò»ç0Ø?á!tÚG‰¬?Ê?ͦ?Ú
ÀØwÐÇ?ÈÙùBF?­z«š\"þ?·@uŽhPMIXED3FGL J1831.7-0230@<u^á6ç@	Ó˜K$ÂÀ7àùx&'KÀ9ÆõkQ‡²?öÉLÌKž@»PÒ@´þh{>¿ç"=ý;ª{¿èóAç½$¿êF$mƒÍ;¿èõM¤E£UNASNone?w-äÄÚé?{<`ùS	[?ÕŶò"¥?ћ(D§°?äï"Úö[<?ѪJ‡vE?½­ŒÀ˜6?Ž4î
( ?Þ¨ã—D?ËÛ2Z	%?ڈóìBÖ6?ÉQÿÒÊ?Àˆ\ÔÛþ³?«ÍÖÀŸ ?Ô
ÉcF?¶BƒñG?á؄:õ±?¶¸@èÚGÕ?Š¯ÄbÌÒ!?écšÿ×-?ÑÔ<ò½?Âêƒ:¡Uj?æ«3Ð<	?Æç¡u—B?S†‡E'‡?]㊬Ö]%?Ò<öó^Sj?Щóã€Ý$?æ×ÁB³Œh?ЬÆÔ݉Ö?ӽؚ­¸,?ÒïXgö	?ٝ¥íºÙ?ËÓÌóZ¢…?Ó)‰¾Q¬=?ÄM‰uµ
é?ijãûE8Í?ªø$sº¨V?Ô!Ám•?´y{¹Ä8R?àÂ|Mû?µ3¥kV\¥?Ðp+Mê?'s
,·j¦?Ò™nÚù?½´q\õµŠ?æ'ñ‡ŸÏœ?À>Ӕ+	ˆMIXED3FGL J1839.3-0552@:S¹EÅ¿‰ÕÓ0¿ À7±EˆÀ9SÓ[\G)@cªpCµ@ûÊ"x{?ù"ü(¯÷¿´Æì`@&¿Û̕asû¿ä徸âà
¿êës§¨·*UNASNone?2ä\w=†?0Ɍ(1¬?áǸ죵Z?Ð5JížÈ?ÜkÕ=9ò?Ð5tO¡í•?-ôÔ ºWŠ?P}"|l;?åGñ0âÔ?¼…•vÁ ?Õl_›•ó?¼ˆÈï{+"?³ÜÚl¸²?yJåDQ?ãǀ'a–ô?»òGõPé@?×ã_ôçó?»´¶ŽP2?iـL´?læ,HÎ?صüíð?Á`láC–?㌯°åÄ?Á¨¬Žé?=øñûtÊ?p©ôFúß?ä0ÊD©Ÿ™?ÐôŒòõ³ÿ?ם7–Í¿ï?Ðô" [Tº?AÞLðm²?`ÀQz'8e?ç)±àÿ?²ã"¡¸7?Ñ£®¬Œv­?²ñ™(é)æ?Š†Ú@ú?Š›?'æAÖ?âîx6%4?¸U+™ãuÄ?ÙNª>ú´?¸çT¶±E?bVý½°z1?kéKmo¤¾?ÚÍeÌÁê?½"›¡`Ÿ?â†ö )?¾$ôý©Ÿ²MIXED3FGL J1843.0-0359c@<mCx$Õ?¦µ¯`À86(ï'µÀ9Éh%ƒGH?÷Çy8¦È@š#WH?õÑÄ ÙSï?ÛÁòu¿Ý˜˜ÊLü¿äh˜pàÎó¿ïÿÕÄčUNASNone1?Q7ˆ2	+¿?W¨Ë³¶?»ýE²ßY?Á©Ìç¸?ìw»…I!ÿ?ÁÁoXtؑ?u®ÈráN?ˆ[7
±/?Õ¡ª=ðjP?Äé;ì?åÎÑ´¾
?̜lxW?§8‹ÒO¦X?˜Ññ‰K–ø?ۈy°3þ¤?¶í´ÖWò?àÈ:jÎĸ?¶‹Ç&V? þnôï?¡"$X²›4?Ëy&ø­.?¾m÷Rñj?èԂ'…Ã?Á‰q
­Æ?I0A8žõ×?UÙŒ‹í?ÀxT˜'9?Á›­´È?ë۞É{«ê?Òå¢~?ˆî
ÂÇw?UGíðØ?ÛòPŽ|žÑ?ÁqÀ›ªÚ£?ᣴÏ]©?Âc–«ŽË?´å>c·O?¡GìÁžkG?ÚUî_ªÆ¤?´ÍírÚt?à8aêµ?´êχHP? P
XŠ?¥èÂ8ٗ4?ÍX£Ãq·Ü?´«Š¨}»?ç¤Ö9Ä-'?ºß&gYÏOTHER3FGL J1843.7-0322@=çáüú?ƍ¥šƒÏXÀ7ªñÀ9À¨á59ž@"Ùz/F@'Ý<Ü@CÕÖᣟ¿Ü;š<#>¿çòµ0Æ=ß¿êmIçՑ¿ïÿAHl"UNASNone?sÃÈ
ß´?yC[Éþ?ÈLïøä‹?ÊNr£Oi¹?éÅ<‹²·^?Ê~îàt¤?SÌòs¼Æˆ?jÆi47ÇB?ád,ÂM9f?À`{jÚin?Ý#ىËm?Àg"CKÚ?³a»‹È?¢ÝLÔrr3?֖øžC"?·Ò)jŠ÷æ?âHLFÌån?¹çníz?‰W¢È$C?ƒzçö˃4?ÞS¹.Ï6?¼Ãumée?àpÄÝ®á?½Y§*ÀE?yëàƤI?Ï–øŸÏl?Ò…b] Î?Ðo²Âç™?æÈw-Þà?Ѓ?,)˜?ièu_֑á?z{©ýëÜ?äÛ䥠R?·¨o#¸?Ö)K—œÙ?·B쥛‹?ºjy[
½ž?¦¶v\vÐ?Ù[MýþŒÒ?µoÊ]†ÃÔ?à	՟aã?¶ÐU:S"Ñ?ÊŒçÀª;?‰Êßë@3?߅횢®?³Îÿ¸O?ߋ½þ¨¼ø?µWu8º|MIXED3FGL J1844.3-0344@<˹M"¿ÂŒæÃCBÀ8I­Ï±ƒ›À:9ºHf?ûîÍÕý£@j#²Œ¯¦¿Û´ÆVø?ï÷sB܍N?Èé"}m¿á_ûÎBÓ¿ìtĚúÝUNASNone?²=Z¬Þk?ÄËúʋÿÓ?ß=úà9Ù?ÑufñUÌ?Ü;5Én&,?ÐӋûÛ5?Š'@b{N?¯á:Æd"Ë?áƒÌgāÇ?Ш½§™L?Ü'-.?6?мîœÅý?ŒP˜¹g?'wG-g̀?ãAOöÁ?·BxN?×î¸ÕtH?¶ß_:fòí?š:ÑS6?¢²Üâ>?ÝWÜÆü?Ð"{-PxÇ?à¢}¤VÈ?ÐyúÀ®Žý?šs#³ðO6?°]ŸÆ?ÖZôËæÀ?ÑèA"¯[?ãÿ\è?ÑÛI"™ï?"JÔ׶Ÿ_?µùT'H?ãcº»Žr/?ÉÍP2¥ø?×óÝ;ž«k?ÊÎO·Uö?¬G¥½²Ü?Ÿý·tw«p?âìE¢e^î?µ»ß(iâ?֞€G?´©‹Á·q?–ÿÛZÌà?žŠ¾ZOI?ږ~íõû?ÉÙq±¯?áüÁ®Owü?ËAKŽ©MIXED3FGL J1848.4-0141@?…fîW¿¼Öpd—gÀ6ã¸WÊÂ1À9‹‡Öùvy@¥cSa|@´Üú‰?ÿSqç£è¨¿ÔàÜJ»‡¿çÈPó¿æv×·%_z¿î"Í]UNASNone?TŒ·'4ÁÅ?Q²¨/õÁ,?Ñãê†Ø2?Σ~…þ"?çÄ` 1l?Ω>cy2W?:\xj"p?Wxܛ†³?å2´Ž=!?¿ZÿsÝZ?ՓÿÅâ;¹?¿[¨®p§n?§1uDo?œÊ"m¢É-?Þ@	v\ŽÝ?ºÃ,`ÂHÌ?ÞÞhÐEu?»œIÓç?v䣜ìy)?t§HÙ¸˜?ÜO<Uh3½?¿µ0'Sð²?᪘Ž
/?À¨ib'?BërÌ"z(?DåÍx¾°?ØÜ­ÿÆãî?Ò¡$¨Uõ?ãŒî#o×å?ÒpúOM?K&q(Hø?e†­–?çsÆ»ˆ#G?±¯ ÈÛ";?Ñ
ßOŽç?±² zl)_?­'ßr:7?¡ÁùlÌ?áTEã 4?·…vîÔ'?Ú<û…¿>'?¸(#Р´?r蔹>]?sb'£3ª?á…rÄ~Û¹?¸:FØ?Ü©x#Óì?¸ŒyNw;´MIXED3FGL J1848.6+3232@O$¡œZ@-| fèlÀ8ãÌґÀ:]vfœí?üÑÂèbÒ@{þÔü?þçÛv]ÕH¿¤\¸råµ-¿éôsH»Ê¿å¸±Òø¿ïŸaæ`,øUNASNoneP?î²YFñg?ªP"³yì5?t,/'x–?z»QI#­€?¢W©±«
~?©¬6*"º?îžlx_s?³n<à?'•³šœ"ù?¥†öےX?žv~Ñ0"¡?§Jhô&"?àýô"¸Lô?µeúïÃô?¡€Žåî?ªuÜ
" "?Ô³WsŒó!?´™ýô`Z?äÒÏdp†À?Å©½[É2?¬UÁt%?¬omöþy˜?ÒÏ©Ggž?ÄÐÒ&96?ïJ×'!_ª?¡%}÷¾?zóÈuo'?…ä=¡ºê?ÐQüûÑ?ž^àg?ï/'œ?¬µgö÷R8?†€|«æçð? 1Åôç)7?µ¾ºÑ§Ç?¡-C[Ô¤ù?á Ž=Eí?´uDܛ$?ÆÕ±zqí?«³^ÙŒ?ÒT
Èt½0?²t—O¿]?è#|ídê?·ÀÓbpÁ?¸SˆLÇQ?«Ÿ^ɍ?ÃHK°?²±4¤çnAGN3FGL J1851.2+0423@Bh"pdìê@d}€^_1À8'­K'E¿À:T\Rn?øè뗾"@1+¼ÇF@šO'ã—¿¿ãŨM!Ø¿ëÄ7Da¿éF	Ï*N¿ïÿÚLÅ´UNASNone?Á©£å'¯?ÃS¦_¦?Ø;ÒF¼Ûq?Î¥ÁkÖÎê?Þï£èc<w?ÑG·/p?™+FW)?ª}28jc?à€žu÷S?ÅåbÆQ?ÝpLë(Ç?ÆÝúf£E?Âà`¤ڙ?©ôK—h?ՕƒM/'F?¶™Íùx?à}&0ì1?¸´Ø¬'i?¦,|²CŽ¿?˜õ0Ê÷UO?à¤{«Ð†?¾}û¡Í?ÛòOqñùœ?¾T*Ó×òµ?Àâ+ÎåÖ´?Áƒ=A~û^?ßS¿ˆt5å?Ïq€¤ïÓ?Ø;*ÞÁ?Ϲš'¢e?«ù?iÉދ?ºbR+W,ô?âFÃBÒ?Â}¸ê!é?×óQÞœÐ?€äZÌÄ?Ò´¨"ÅZ¤?±Þo'9L?Ò.ÞÓh%?±R–šž—Ô?Ûx—Ò€Q?´P'HvÆ?±Šg2 /? 1ÛZ´Jƒ?âPÒòÅs¬?µmã6Go?ÖûÀSj\?µ¶Ò=
ÍTMIXED3FGL J1857.2+0059@A<YÈÉ2¿êçLàƒböÀ7À!)Es¨À9wúÊ6˜?úSÀý
Ø @.…fîW?õRtK×Cô¿àû[4û¿ß£†ŸcT†¿áNnokÀ¿éE1çwcUNASNone?UÆ0¨ìT?a<¾ [p?º{`Vyp?Á6l²Ÿ"È?쥰ð'«?ÁIb™*Ô?¡ŠçV'?¯'Õû«¤·?Ëì'
¿?¾w"°þ?è ñ"Å^?Á̀¿¶—_?­©^+:?œŸð_säñ?Ò~®BkÖ?¶Yu®ïu?äæü\'?¶óMòƒ?§éŸô˜?¯(«uC?²žÒ¡I¨?¯Ԇ&6?ì?R3å›â?»Rïâ·«å?M_CO'?X_ÍVEÃ?µe-hÇSa?¾ÔÙ}-ä?íL';Y?¾÷áÛI3È?´éÊÐÇxè?¿ýl
*œ?Ñ_&ƒCä(?¾ÄdÉXN ?ä³3d%?Å=xe?µó­Šý`?¢±µ¥UôÛ?Óõd¼Hh?²ßЏ?ãFØHãñ?³s˜'ÐÄ?¡è/kñý?®~y2¿ò~?ÀÝ#k-å/?²$´©æ#þ?êª4.ZÜE?½ˆ†™.18OTHER3FGL J1857.9+0355@B•Î|Ð57?Õñ÷(ÀéjÀ87¸Óñ"À9Ü7i"ÙI?ûMFˆï@Cˆ?ÿõ?úÆ3
nmò?ïšÞw3#¿á•¿Ù8/¿êºÜÓç.‰¿è"HÒõ UNASNone?jV»+BVš?lÔL*Ítm?Øz±&~?ϱýô7û?ã¨P±üÅl?Ï´ ½~"õ?ù!
	µ?•ðëȸ'?Í"°¬ä,Ã?'CV8hI?èooP3¸Ù?Ã	‡†OB'?­°Reúñþ?j"Òuª½?ÑËÁWNÓ?³¿ÏKGË?å?-ígç?´Ç|3Ü? X‡QSÀÙ?šˆ*s?Ъûƛ—?À'Û½´¹?æ¥mL.W?Á!¹ªz§?k{©ëµ"ö?t§Ïšåý~?Õ|ÆÃ&
Ž?Ï¿ru'&û?å& ôtå
?ÏÔkÿ¤Ý½?"rÒiö'?ª®ªtsŸ~?ÓÝßµ˜äÏ?ÃÊiK¯<)?åmy'_Š÷?Äσå—æ?·¶gÜÐS?£²ûˆžy?Ô?E˜Ä?²>u­ªha?ãaÂÎØ?³BO r¾?£^sVMa? {ÿ ?ÑÊ%뉱?¶`œæ¿·ò?ååÕEÛñ?¸ÛSßÏS¨OTHER3FGL J1857.9+0210@AÍÄupÅ¿ÝyO܌À7iKB±ÂÀ9³ŸAyG?ý­åSViC@dõOÍÈ ?þ=Ž@u"¿äf©#Ǩ¿ã3"]¼¸q¿æ÷ègï
Ñ¿ìÕZ›¾CUNASNone?E8Õ.å¿??·"[DÚ?ä-þO©õ?΄dچZ?יf÷cã?΄MCÍÇ?S¡(dé/Ï?jMáõÔß?ß33ŽwÒu?¿Œµ‰Óí—?à\•¤Žâ~?¿¼ñ€"ìº?šyl̈¹Š?ŽrøÊn³?âÝȝ"#^?¹E¢¥]§c?؜×÷£:,?¸òSsÌSÌ?Ÿcû*—Ô?ŒåÆIÏ!©?Ôº?kû¦ª?»¶;œJ?å$bº#@¼?½N-[>%f?3Ã趸Å?3T̞Œµƒ?ä^>	ê©?ÐaÏvRö%?×?Òس?ÐaiVÛ®è?e+ãS¼¥?|JC²g´Û?áÁª¥±Á?º[	T<˜?ÜRRïLdÄ?ºò‰
Êä?¨ï¶;"Ü?š†çmësŠ?âüãY<m€?µ[w:˜.?×;Vöºe?´ÇãµÅ¿Õ?ŽùeL¯?»¾ìì%M?Ø0€¤2ØM?¶¬,û•õç?ãm‡È5ä>?¹mh @`oMIXED3FGL J1859.6+0102@AeUÅ.rÚ¿õ¶âdä†'À8
šôãlLÀ9ј:ôÉ?÷i§¡D2à@éüíÑÕ?ÿ'%Ÿ í? I^Ó&¿ãoòÿïíl¿æJÀŒ¼UJ¿îŸØ"UNASNone?v*´6»lj?uÃ-ÞªÜ?ÓDƒužpL?˔'R@?æ1hÜsš?Ë´'³çèK?§óûüû?¶XÄÙNÀ?Ñ®•ê}?¿·H@¶~'?å©uKJp?Ãáý
­-?±ªAÿÌö?¤ƒ®c¿½Ò?×&ÛõÅÑ?¸
£KÐâ&?â7¬R™?¹±4ø§"z?¯{ãÝ&å‡?ª$¡`g'Ä?ÿ+Ýq‹?±±ÃBÁ¡?évü-/?º?Ò,Ký?{<ƒÚ»°ï?eR"koI?ÔÌø©ýói?Í°ÅÉèÐ?åc
£
öB?ÍôUìŠq!?¸ˆÏEBÂW?00/®Õ?ÔIõ³\ ?¼en]š~¶?âÉë=rž¥?ÄîêYƒ2?Àւʃ^?©ÑÑ|0"v?ÔQX†Ã—ß?³¬èž?ᡳ
Ó9?¶Z!"gó?°ü¯›D²?°2Wb¬?ÈÊyÒ:09?ªÂ2Fҋù?ç­ß•ëþÛ?·ÕÁ=!ž‹OTHER3FGL J1900.8+0337@BœæB¿˜1¿Û£Òm¾À7°]«¬Á•À9ñïÞIÍ?þ9ì$ÖÏ@›,ªØÜ%@͵^q$…¿ÓfÙJVê¿êt–Ë'–ô¿èèæç]п/âØõUNASNone	?S†\Ðæaô?Q%üF?ߌŠïÕú?ÐÇÆa½y?à/÷YñÁ?ÐÇ>í?wÔ?G	œ¼Ã_¸?bâç+uâ?ãj\ãòƒ?ÀHe'‰?ÙÁkÅ ß?ÀKyäP)Â?­ò?µ
µ?žh¥Ê™0?Û¯"gƒFò?¶*êwH/?àIÐqÙ?¶ÖعF"?‰»`ʸMù?'uGð!˜.?Þ ¿LJu3?½^¡ÿwL›?àH²Öxêo?½ô>ךö?8Õ{Åç¶ù?<æâ|?み7/c'?Ð螙!"g?ØöL22­&?ÐèŽpÙ?Y+‰À»v?s[»Kߘ?äÙAmwl?·ÌCê)mÑ?Ö3þQK™~?·ùgë ÊÑ?µjµj˜j¿?£rÔ£yÏ÷?ÞÑTLn©½?´?1ÔÝi2?ÛÓþXϾ³?µ.óLv"?¶6ùµdÜ?†æÃÏò¸?áÕ!cÁµ0?´:1v'ú?Ûha?´þ±üÈÛ)MIXED3FGL J1901.1+0728@DXÁTɅð?óþäǕUgÀ8.üóEºÀ:8*ù?ù霾è¼@
Óô²š@}…¬o	¿äen¿æ›Ž^RÕ¿çnÿ¿Ø¿évPŽã³UNASNone
?{LÀnâù?Œûë74ä?ÃÇ°‹×Û?ÃMè@F?ê×z\+hÓ?ÃPDþ"!Z?¿¸#PÑ?ÅŦ)—J?Ìõyîê•?Àáó‰"ÖÑ?äá©£²€?Ç¡¦½]\ì?Á.ÔåÜ#"?©bà"~ªâ?Ñ~€Rd•›?³–S:¥óc?âõ
V¬N?¶?é	?³ÁùLA(?¬L[¿—¥¼?É=©TˆÔŒ?¸·âô-CB?çM½kÂ(?¾ {¾šãy?|ý¶*E7:?¼É#¾ÙÂ?Ç»üE
v&?Åÿ6»lÁä?é×'B\h?ÆcQbb­?Ôò4oA?Òô,áúZ?Í ½û"ˇ?ÁûÉ¢Ô^o?Ü}l'Oxc?Ìg0E˜¬?Ë='ÔøQ?®sšÐ}Þ?вj°‰í?°ÛÔrJ¯®?à×f¹r|õ?´m–n\x?¶'ه"`?¯BdRµ»€?Ó°ñ"Å^?´lÏþX֞?ã§åk÷lU?»÷o€Éò…OTHER3FGL J1906.6+0720@D˜±_ˆü"¿œ6‡P–ÆVÀ7îü¢}nÀ9áa£‰¤@'a–óÍ@
ØK)tª?ü¢üSøû¿ØŸtùÀå}¿âhÃQ46O¿ãî¯=B¿ê"G§"]UNASNone?Uͧi™'?[¨g[¼Ö?â^
€??Ï&€C"?Û.Ýú'θ?Ï#¤NBG?2˜hsú™—?UàÁü;Î?åGï¾ûd?Àþèì?ÕúÊÈ?ÀýëCÁ‡?"uµœï?ŠÕ^=cgø?áâ
.Q?½Eøv"Â?Úó"'ʘ??¼Ôƒ¡þo?y-ƒãþ+d?t&@~Cօ?áY£¥ZS?¼ë‰»Ö"?ÜèËwÉK?½SUU™Ô?@,*Û?EýÏëlRG?å«I"ÙC(?̀ª·p'…?Ô¡`à(?Í…£Ø?J/%ÜEǖ?bgŒ/¾~"?çTGŒJjv?³ÌLˆ(½?ÑJYUëÒ?³à7ºÎ¿ã?¡àÎä'?–6Þ#çYÏ?थ«¥Ï?¸QreÏ?܆x³¼°?¸
_Ý
ÌA?z¬"ª_"¯?u j›¹¶C?âÒ%l 9±?¶Óf1÷Ä©?Ùñ'À:?·s–Y³PSR3FGL J1915.2+0954@F9q!«K¿æ'"€zä£À824Òo£ýÀ:3î*ëf?úL0':+ @TYsŽÃ@Ú1'w¿ÕZ8äD…¿êÀ>/ÕI¿çÙŒ/n¿åó¡:!ä×UNASNone	?zâËG±?|ç}çKh?¾À#,f ­?Á´Ï—¤Ä<?ëò6Ù9©?ÂîH
K?™·íΗU±?¥†·Žž?É|_èÚÕ?À;†Ø"&?èÓ(—+ˆÍ?ÁócÞæn£?ÀÛÃÂÚR?¨Öó»O×?̹éìÔeY?±é-1új?䚿Ú0?µ'›®Ð@?¹Š¿~^?­SXÏqd>?È6¾´liò?¼_CX*Ÿ¢?æÀøc‡"?½«9™Ò?'þOK£´©?‡ª5†GG?µfWš«p?ºø,-ý¶œ?í;Ïu.ç?»÷#K½ ?¨£ûIòCR?³1'°;J?Í`ðâÞ?¿jûáã4m?ç"Òc?ÄN‰vœûŠ?̟´tç3?°B~üEœ~?ͺr=p?®ñ‡†æq`?ᗸc¼Æx?³â8·rÉ?Áx@'†Í?°!Ÿy6à'?Ô?ƾY±;?¸£¾ S?á'{¨0Ð?ºßS74ŸšOTHER3FGL J1919.9+1407@HZåÿ£¹®?Îó_ތè±À7Ȓ¡WÓüÀ9õ¦gÞ5«?ö{ëV¦@ܲ_Ž0@|®fÛ+_¿Ýº}ºjõl¿èR	c¥¨¿èqþÂé<¿æNkwQUNASNone?…ßáOú?ˆêS×~¾?ž4`èt´b?¢$òf…K?î¶àØ®"?¥›ŠÔg?¢ÇÄILxt?«Ér=J"?½ä'
i?¶ øóò*ª?ëKRÓ{?½ÍÌüó[,?»nJ5ƒE?¤î
öI:?Ɲ[ùƒ—­?°º¿‡¹v?æè»8Xi¬?³¸~ƒ‹?½Vûàò¯Ç?±µèL){?¸fSØ*Š?©ÝéYê9í?éQ³¹«\æ?¶ÆÅÁ¶I?A¼¿·±? Ad÷–óú?±~&gñ÷l?¶hYÔ?ìæ-MŠ?º*+¥1?¹+¬Ç)çÞ?½ûuAJ£?Ä|U»ô7u?·¹øg³?ç»tøFðw?ő°I¼ë?Ä8Çl'"?ª'ãaÉ$ ?É
Îs.æ?®·ÞýFªC?䮊¢?²ÄyèG~N?ÃtˆÍt?µcT'{mT?œbxèk†?¥ØW[»Ðl?æ{Å/
x}?¸¾èéÂOTHER3FGL J1921.2+1506@HÝø>Ÿ?Ûi' hÀ86uT?ó5À:V‹"ÞQ?ÿ̒_"Žh@ƒjY5@´s0T¿Ä7·sÁ%¿ë§äO‡¿î•Uël¿îfžšŠZaUNASNone?{ü^™î&?¡ð5Ö¨M$?ß(聉,?ÒùaoÓð?à3"%Ê?Òý[¿ˆ/~?PéŽ'aJ?g<¶YÎ×?â3÷£¦?ÁùN¦èGä?ۈüƒHÊI?ÂðÕ–Ò?³ß'~_?£¯Xø³"?Ü%½Qç?¸^ \@ó?Þâ{ü«b?¹ƒSc?ŽÓŒEç?…[4²xÞo?åFƒV%{?¾áC_ÂU?Ô|\óÝ0?¾*†Þ£[?Yë®_‡y?r?n/ւé?èmºZ³Å?ÌýQÀÎ"?ÎÂÕ} ?Ìæâb5TK?eóz~Ú?xd~øã?ãªv"h'?¸Ý!˜Pû7?Ø-1\³?¹7²ˆæ´y?Àυ
ñZ?©š;ä¹|?ÝÿrÕI6?µ+MuN—°?Ùõ%hf¾?¶!õs°?—
¹{é?‰B€Àö#?æÆ!M"ÂÑ?±tKœg~?ÑŒ¹®¯M?°Ügú""áMIXED3FGL J1925.4+1727@J%]Äuq?äp?ÎL(ÍÀ8•+á/ZÀ:`Þ	53?ýj0'|G@Ûtä®jâ?ð¡ç¹b6׿Õ9n€ç-¿Õêߑt|¿ëÉ7»qõU¿ïÿâ–b­tUNASNone?^ Ʊ™,o?c1'kJ?åiÎÃG
?Ðמi"uh?ÕA²ãþ©?Ð׿Ϲ;K?k¶H|÷œŒ? ¾ÝG"©?á´y!‡˜?ÈcX#|Í?ÜÉ*}¤gö?È`ÃF2¶®?ž–e<Ôe?'Íwx¤¯â?åCpuP?µz²x¸£u?ӏ¹'(tú?´´÷ޒTÓ?—Öò[âÿ?•Œ«3DÜñ?ä×jbIvA?ŕl:ˆ3?ÔÓ¼֒/?şQ¿e[$?Wt)Û	=N?fA$|Oö|?〵-ãß?Ò´[—*~"?Øç!z®õ?Ò³cÓÆt?"7z^?–0"ö¶bû?ãŠÉ;$ç?Â& Þ?ØHµàeõ—?ÂQ²Oø?§Þ'ê´ý?›©f2'c?åë‰ÉËn1?³+¦c]q?Ñ-'oI}¼?±÷2ª`áù?Ÿý;¡ä
S?˜Ô^dD?ä´T^a'?½Ôp3ˆ‡g?ԗ"›‹È?¿	'÷z0¯PSR3FGL J1928.9+1739@Jm[[Õ?}&3ò"'À8imOŽ³À:4››ÒXþ?ú@ÈÍcˁ@òlÃ!Ó9?úgRژgj¿á1ç)€"¿åQƒ8aÎÛ¿åÇ[sÄ¿íµ²ÔÔUNASNone?d}c"Q—?a\œƒnâô?Ô¾Šêª-f?Ì˞}ÈÇs?åŒ='J>4?ÌÖ
RÎÙí?s<éOBh?†Fd*Up?Ô;kæØç?Á
kÔ9}¥?å»Ð:6ÿé?Á±HqF?²ÿ)jma?  ³M®?Ül¾ÈZÕÂ?¹wÓ2Åä¡?ÞÓvÝày?¸Ô"¶%²?­H~ž'Ì?¦ô"ŒÐŽ?ѵÁ ?½EێSã?åP—ŽÙ¾?Á½©)•·?bh"pȶ?e+#º›?ÐoÅ
Þ¡?É[Fç_?çµµOòJz?É$¤ÚÀUp?‰XkÂiô?žà±í3°Ã?Ù$1b¤?¾<ËQ;u¼?ãWŒÈ'?À§,
hã?ÁÉ¢q•ª³?¨Š—JÄPP?Ù»"ïCwØ?µˆԇ*?Ý_™×ñ²Ï?µiŽs¯4?°r9eç?§‹‰VW/?Ù¢iÎó#?¶½_ú5?á-\ÑV
B?¼0ÎKÛ~OTHER3FGL J1946.4-5403@u~6z—À=ûH
[À94ìð{(À;µû-2h2?þρËDz@
r©rՊŒ?ø·÷'¿7?×¼ê×yÏ¿à܍¸'¿è½ãJ' V¿ìýco³c'UNASNone?wæ'%v?wÛ(ž-?ì!
gÉ#0?ÀÏz©ip?½yC°%nœ?À›i½ÞÈM?‡IW«Æ>?¥rÇ4æž?ë6ðiV}2?Àß*_Í?Á¯¨àŎP?¿pã?©ª¿ò
G?™'¬^{?ê¹ÊÊû!°?«\$ôûë?½\JR]?¦æ¥ðLÖ3?¤Ë`"~øe?"O7É怍?ìc‹PçµB?ª&AtsØ/?²}õ-8ÿB?¦ølGÐ?a¾¡éÜÁy?güåwø6î?î[¹ÖK?²\pÆÌ«?©(x~¾?²&DßV\ñ?˜¹º1¥Ð›?œ~‰/›Š?ë|Jm%a?¾Œü8†jy?ÀÒב)''?ºG6qv[?³ó%Øgñ½?¢1
ÆÏÕ?ê
Ì×è?­n–úl"?»žsj}CÅ?¦Œ™;[èâ?½ÕÄá#¤~?¡=‰¿"?ê£+EJ"U?¤²-$«yú?ª!ÁäÄî»?š_6,þêPSR3FGL J1949.3+2433@NšiƒQY¿çCM\ª%À8ÍSù|X@À:¬°',ãŽ?ùƾ•|@
ï/"Ã?øâÞ0¿Åçö-z¿çnKŒ	Qý¿èJ6F°_ü¿ïýÌø$ÙUNASNone
?y.cûR?ƒsUøú?Ão½o.?ÆèÓØHš½?êñ³×»ñ¼?Ç[1i9?Vʬ¤ÌÈ?pZ¡ÙÓtH?ßú©»?Ãýëþ–H?àiúE½	Ç?Ä'-#à?¿Ùëak"?©Y!2Äg<?×Ñ·æ"Qº?¶wK-à??àæ¡æ?»G<·bÏ¥?¨à—aÞ?š¸\E+?áuuˆ Ö'?À+ÜÛ@a?ÚØۊ ?À†ÑDD—M?Ž@
86&?–Q𛤅?Ô[ -m³?ϘiÙ7"A?åYyû2ž?Ѓ®\Ÿ?rËaUðùX?ˆû‹££ÿ?á<¬üwà6?¾FÀÇj°?Ý;x'ƒä?¾þ¡èêÜû?Í¡ú?}€?®ßok]?Ù_|Zw"?²D†!—ªV?×φ…ÀžÁ?´JâJ!14?±ø«nö[? qz~'Ïx?ã™Ì#€2?´¶á¯n(c?ÔNbO;¸¤?µ÷2:G¡MIXED3FGL J2017.9+3627@R¢ª:э&?ÚIECVÀ7tUóQ›ÔÀ:1GNs*š@A(¯ ¿h@
{œüOœJ?ö"|ôÈ>s?áô3ˆî{ž¿ßå: &)ú¿è§°[…•^¿ïh]QóEeUNASNone?o	''Ù?KýVl[?ç5A¿#R&?ÌM¶c¡1‹?єe†(+?ÌM¡~?v
?$ÿí¼ˆp'?S§tÒP¡ƒ?êšÖ;Wç?·òqh'?Œ¸«úçŠ?·êxžì!£?t!ç¬Ý#H?pœ4Y?ꪽÕ|ão?¯ü_¤È´?ijùl=	?¯³ãäÛí?TÇþï¥8
?Rv7?ãiú?ìZ¿^UK?¬^®×±fÇ?¼Öç(©ÓŠ?¬>Ãl>ú™,;ù?(ºî&'¿?腙'Á@Û?ÎIœÅ⼒?ÍèÈÐWµ?ÎIy_3¶?C9Â*ɸ‰?e ç"®?êþöÍs³"?¯–Ê{Fš?Ãðë»Õ?¯Su*Ëò?tñ©ùש?|ÓI2½±?ê¯ /Äê?¬ÍW¦Îï
?ĞøY©¥¼?¬gèvÀ^|?^psŸ÷7?Us噼?ìŒÓ§KM?¤Úg‰äá:?¾ÙØä]7>?¤Î+¬ã»PSR3FGL J2023.5+4126@SÐ:>À/0@»|,ÑðÀ8"Ð=1À:pñÒ?ÓU@hòbˆ‹@ ŠÒ+†l@BMec‡¿Ü:&ôØÑà¿æW?ÁQ!¿î^måû`οأ>ÍUNASNone
?МNL5°?ÌGg"?ÚÜ
ûº(¹?ÐfÄã§ã<?ԇ¦¶ýF?Í*vù(í?Ó×x9ò?Õ\ՓšÑþ?Ê+´"«!?È{÷$í¨Ã?ß­-íp~?ѺÕcŸ6¼?Ñ¿9 ww?³y+×?Ó'»þæ?µAÿu8?Û)ž´ás£?¶€B®.?³T
ÅcŠ?°òtã=?Ùñú…äþ>?Ðn9û4¥_?àœnÆÿ?͕8.$Å?ÐÚ£%DÄ;?Ë:¿n•_?ÜAÜ?u?Ί
>Œœ?ÒäMÇÞüO?ÌcZå¡&x?án¹ª?؃'M"{?ÅÎI¨ÚC?È£ØütÉð?Ò÷þø Á?ÐYÔ®SÌ?Ø'4f'ëñ?µ¼Ç)À)?Ô?ÇÚäV?´[ÙÛk/«?ÓȋÑý/¸?´‡:I"…?¼`¯Z9²?¯ð64:1?à•‹áéÑ?ƒÉpÌÆÃ?×¼¾eò?Ãc@'sžMIXED3FGL J2024.6+3747@Säy'¼?°«'¡Æ3À8¢×áÓÅÀ:vXò	8?ú*W‡PkÓ@MjàɃí?ý©£A«q?ƒÆó¿ë ǾΏù¿á8ÌÈ5‹¿êú¿»ä"ŒUNASNone? ¢3L:µ? nò?ÔV?ÆÁŠúD?Ƈôž«"Ü?éq›_†<3?È^{$R_?ƒ‡¿ëՉ?•Ü;Ðqº0?ËL,'>=?»µ$¤úö¬?èÞÕÜHž]?¾w?½WÓ?ÀÒé´£?¨Á=èçâ1?Ô»
"!Â?³_zø!lë?ámì¾Ém·?·ZÙ#Œ?¿( eÄ3?®öO®è+?ÊfažU–
?¹µEÊ©K?å"â"]á÷?¼—dn¬—?ºø
,ä9¦?»}œÊãt?ѼɟpÉ?Éu½DL=Ï?㙊«@?Í_h<̱?šÊŽÊ?¬'‹#ÒEœ?Ó1½ré‡?¹èƒÙá)È?åÐê‹?ÀïwféÃþ?ՍË3‰^'?´Éðv
£?Ñõ'…xFÛ?°'ï^ý`?Ø|²Eëz@?µ.§ëé^?Ãèª)µ?¯£Ø2—¾?Ùxsâ®?´ÛÛAžt¹?Üì‹|~w?¶:	ªèOTHER3FGL J2026.8+4003@SŸ}€^_1?ðf¬ƒ§ÀÀ85>˜ÂEÀ:S½ei?ýöâõÙ@ð}0Ò?þ̌ÐÞT_?î´®>R‡H¿ê³¯J¤Ð¿èÏÀG¶Öt¿æQA~6UNASNone?²ÚÌ´K?´\Ùà0¬Æ?ÓZžÿé?Ѕ¼ \R?äy•yò?Ñ5ߟáv?¦Hw¯ÌÒ?¼P»]¨kˆ?Ïi±úÓ4?Å&Ғ3ž¾?æÁ=¬!ËF?nj	iœb?ÄH{€@ ?®,ÀÚÿ!?̪ӈ}½p?±-½ÄÅb?ãÃ,=ÜÀœ?µcé­òÛÄ?ªÅ{Ô™Å?Ÿ@E¹t_¶?Ӆš#,Tó?êåúÎÆU?äÛ15úZ?ÃFÎ4o¸?¸Xx툡R?¼ƒZp—u?ááOU8¢?ÑÕâ>gÞz?Ö'CžüI?Ð×û\`?Á×ûVD|©?̺àq>(?Ò<]¼§CY?Ÿí
É¡c?âkÒL¤¯ˆ?Ê®4)ìý3?ÎÙ¦á^]?²ãßO¨¬)?λ
‡¨?°µRX斺?àĐå¾i?´‹¢ €òç?´Â}'°äˆ?£'•PyR?Ùj¸tiù?½GÄø(?à×úÿK`b?¼¯ÓHšMIXED3FGL J2026.8+2813@Q5éÍ³}ÀK5°»õÀ9˜d
ƒ À;:†œfÓt?õà—Ê·sÊ@ᓿºëy?ùj§ŽN⼿â2kü¿Òs=idj¿ï†)ñk¿ïýGwtUNASNone?¶®¶É®žß?Âã–Îõ,N?èþßò‹½?ÉlŠ¨÷?À­$ÓknÛ?Á8éE9¬?ŽäHXM7Û?œ'ÒïàÿÞ?æОq"`?Ãÿ©¡'#å?ÒÏ<€[Q'?Ãsõ#?ÌÙ'Ûބý?°&ñRú]?â	«cVͨ?µ:ò*"•?Ë*–ÆDa?®Š
¥zC?®syW+vV?¥x'¾™?ê 5)­x?½m'uºÂ3?ÀF ÖØG?·8YPOäõ?½'@:ò^?Â=Ñ–W'?é–$[Bà"?ÆvJxãÛ?µÌœì®kB?·FÿPQ?´¨º§Ñص?¼ðÆÚ£Ö?äN±à§?ï(lA?Ò8m"Øê'?¿7§Oÿa?Û°/3Z†š?±äþ=U?Û/À	ù[ª?°îßû‹x°?Â@!‡}üõ?¥¥åEŠ;?ÄQŸÉ£;s?­ƒE{Qˆ?æÚ6Ú¹J?µÐ 4=?ÀE‡úñßg?­7zqœaMIXED3FGL J2032.5+4032@SàÞ~¥øM?Ü
#$G]À7 dJ,süÀ:*†ƒ<`@÷øµ"@;U«3@˜­×êN¿Û‰å—=¿èÒ~?ԉã¿ïÿÌÔY‰?ïÜn~Éð¶UNASNone?ä̂ð4ÛÕ?Õ\$÷ŽË?žªØF­­[?¶A¬!y1?Ô|L›}ä ?Ô%•®×ï?Ù	ù'£?Ø<'M¡É?¤9ƒp—ª?ª'£S?â7k5Fø|?×'ø6ÝâŸ?ՌÇ$tÿ?¶ÙÆ߇k?ÊÌniPaÓ?´[jA¹Ê?Ý
· yX?¸ÌâcÊÆ?èä,Ԏ&
?Ȳƒ²žñ?Œ ož3â?®†Â®9.?Ê]¸žRÍ?È,z?疗)¸ò6?Ô­f-dä?K|ãÒä?²gG–Í‹?ÏÐ늨(?Ô#ì¸?ä›O*ÎO?ØJ'¡.¹Q? ¦âi'Á?£ÁÛ¡ä²@?Ô´…ˆ•K?ÖOZ¾	?×ì:3`2M?µZHJ…›?͕Xäȗ?³B	9å~õ?ÙIB -ig?¶iû¹wÅ?í—Jƒÿþ?´²ì
¡{?ƒ )`ä€Ï?¢c<gô·Ì?°á¦µ4Jx?²ãZÉÆMIXED3FGL J2032.5+3921@S¤´·,Q˜¿Ñ0l娶À8,Áúá³À:T
ހS?þ/}Ç/%@3'W°ëñ?ûÛ@bƞµ?ՇW€M÷¿ä¥fÁÕøÅ¿ê`*èêmO¿çºº•VƒUNASNone?¥t\D	ÖT?©¨&‹k>Ï?àÃöš¯ ó?Ҙ˜–þù_?ÛɇB©ó¯?Ò(y†SÁž?i3£¿7
ø?zݱsmq†?Ӓ±:žŸ?Äb"y€/Ì?æs¿{'­?Ă
†Á¥§?½:ÏðÔÐ?§ÕL½¼ÇC?Ò-Pzì°B?´ê™n)?ãFh‹E?¶/'à_>?¢¬Y<kÇø?˜;«ÖÐÍ?ÛßJ0ƒ^!?ÃÎX¨k?àå•S—_`?ÃKsBî<?ª ×P‰Z\?³!a=á?ç栒©‡Æ?ÎIÔ"?ɽGá7ŠR?ÊoO4+çÌ?ƒœ\™=f-?'x!`:?×\ÀË6ʗ?õ"nm¿?ä.("T?Ä5g¼ö‰?Æc8z¿?°+œF¢DÇ?ÔaËdËdK?³/å4x?à6L.ú
ë?´µ©)£u7?«[ª"b\j?:gž¹'Ý?ßµ¹ò÷Ñ*?¹0›á?ÜÞÐÉYé?¹h<ظ
YMIXED3FGL J2034.4+3833c@SŠOv_Ù¿ð®â5ꝘÀ8^ìÔªÀ:‰Ë—B§D?ú&ñ–…½ð@›àÆ©È@;¢F¨0¿×¯‰Uw¿ë
¬ÑÚ¨®¿ë †?A*忁
cgÞ>UNASNone4?°ç½¨'fè?±ˆ¥"Öi·?҅`gñX?ÎO"+µT?ä XÌ­÷?ÐÝÐøwî?šÌ6FZz?ÈOî*t?¹ƅ_û¾?¸§¹]}`]?è6""?'vaõØ#?ц>FüW™?³ôv3 ÜÓ?Ë×±4ô\?±";Gxœ?àFôD½0?¸%'r8k?Ø!ôžšVÐ?ÅE+:7Ö¨?·,''úv?À®æVzyÞ?á	skTZ?Ç!€KrwÊ?Ävf8ÄÆ?Ãi¢Ïq?ÐtÌÒùY?Ê?Gb.G?âÓ,e}¢?ÐjŽ2wp?Ðêy}fÕ?Ò/ú9þ¤?·ílÓE•i?±K°ø}L?äõ]("á¹?эcUdáV?àœìœ˜I?¶ov
L?Åþ6$1ì?ª¨à8®U?ÓÇ´¶wî?³j&RÄ?ã7ÞS2/?À AåŽÌ?·¥Og«¼°?µ®wïà)?Ó¦ï̋V?¿Æ–ÅÝMMIXED3FGL J2034.6+4302@Tq?l&š?ù¨·^¦~"À88;·f3À:bþ;â?ÿaºÅc@
ÉY;°…C?ÿ¾–EÒB¿ãRêCçG¿ã¤Š÷t¿ëpK&L£¿èáX'€_PUNASNone?ºï¢G?ž¶ŸÊò=[?Û؅0ð§Œ?Ðyô–H	?áœÑ¨ºÚî?жpüJÙ?šBˆc(ú?¯òñՓòp?ß«•a÷?ÇÒHä¾?Þ°BíâØ?ÈCWÿ¬"?ÆVš1€;á?®-·3³a?×q¢C%2ƒ?¶"äïså?Ýc¤¯Œ?·Ò1?çA?ŸÅ1@øjK?–Ì; u=?âÚÌn'?èô€oý?ØNÏ´¢x?¯¿ ¿S?‹ˆfm&±á?›Á†mxñ‡?áì£Úî¬?Ð	åúù¹s?ÛK£" 'ú?Ð1©"ÀD\?·'_€œ‡0?ÄJtzÚ?à9}ý(V®?ÅptÎd;?Ù¨¬%Q7?Ä֑¼Ö_ž?ÑUM̈ü‹?±Å£ż9?ÙÄÿ·zx?³?˃Ìì?Ôå³$Òi¼?³8D3'Ä?¤iº-×?•ºU\ðõ5?廃*䧁?¶ÝÜÈ ?ÑûÂdz9=?´ºY=ðÒMIXED3FGL J2035.0+3634@S(ˆ&ªŽ´À†»øiÀ9°à<4À;
-åìY?ü«äåS@²ìì§Þ?ÑNÓã:?ïêÖò"[3?™é¢à.Y¿Ö¡CU®÷é¿ï0#ëËUNASNone?†suØ=0?¡L ÔeŽ?é-Ô?™X?ÎÞ÷Ç¢A?Éáw¥d9L?͆È.óš?|DzUI7?™´D&Õ?ãŽ1þÍ?Ì qäHê?ٍѲÃ>â?ËÐ+X€¨?´HÌñúr'?¡û%Šw??ç?鵙]?³œRÔGÇ=?ÈÛò¯Šq³?±gõÙF¾ç?Àà iA?µ±'äT¹ý?ãU(eq@V?ÇÉtªÄ0¾?Ðå_|¸É?Äh7l'ña?'7Si¹¡?¨~ºYvˆ?æ¬ïrqÀ?҈§5…ë3?ѕ­¥®ê}?Ò;y·Àºß?¾c†à?­qÀâˆËÁ?æÐdr?ÄcHƒÁ/?ÒÚy L]ž?Ã,Ö܉ó?¿Cü¦{¡®?©F^Ù]É?æöË"þˆ?³"—~XÂÜ?Æ^&€65
?¯ÞÀTTâ?ĚÇæwÝv?²¥R÷¿?åbü*¢.Ø?¾•¬1HC?ÅÙGnÿg)?¸(^| ݧPSR3FGL J2038.4+4212@TaÄØì–?á]iR‹¾À7ö;¤ñ¼pÀ:ûwÛð?ÿSÊ7F=Q@'<§P;'?ýC7àlõ¿¶ÕA™(¿åæà/'N¿ç°—já¿é8‹ÛÀÛUNASNone?`p_.PÚÀ?`¼f¢Ê8?Ã_L¥¹Ò8?' ®-F×?ë¼wjÏ?œùïßeE?x°6¿[×?ïÐYŠ?ÙÈát"i™?Ã{Ú¢‹
?âëYåFÌ?îï'{Ö ?®Œ}ñ*KÄ?žªdÝ?ӟÀfÚL	?¶Tn´l{?äGWíI;€?¶÷‰â2ç?žú5œ·4?•W7ã8–?×q¸Ù>¹é?¿F᪙5
?ãVûÁÏ:2?¿¾òÞH9?TÀÅ}_ï?U˜Kèk Ñ?Ò'@iZ??ÊQd9$?ææ‹ýF3¸?ÊÓa;";?'9$¾ð#?¡,6æWH¢?ß
É\ªÐÏ?ÀOôëW…?ßѤW¸£ ?À'=WÏJ?¸!Ï¶Q¯?¦Eç?ÖŽzE…4?³yÉ (œ/?á숈"ü?´ÔG£? dŠe–?•bÁ•÷?àIɵô¡±?¶é6RtŠ?Ýk`Sz.?·ðÂÕ"ëMIXED3FGL J2039.4+4111@T5¨mqó¿Ê'¼£nÀ8û'²õ‹À:AàLÜQ¥?þìñÓA†@…̘Ih@ê:Ì.Â5¿×´È\ƒAF¿èPÎáÇR1¿ë58~v¨~¿äÝaeÎUNASNone?côd,´n?e²rš-"Ž?»Ã܉ê`B?Â!{^ßÎ ?ìs`_ç?Â>ºnq?|%»½¼&Í?ŽŠ0?ïÌZ?ÑJ\Þ/ÿ*?ÃÖ^Ø
ÙÄ?ç"†ßúý?Ä;±è?¼–¿¡Z?¥Ây~?Ð6ËKËä?·õBð՝?ä`!Ú+–B?¹3§(KÄ<?§òj|[×R? yƒ­&ÇÉ?×øhá.ÈY?Æ2DãVHƒ?ℤç¢Þ^?Åњ€¹?eÊN¢åD«?nþ]ÈÅòŒ?¸·)ÉéGÌ?¾Ç5ôƒ ?ìÓPxN¬r?¿kê"·Õ?ƒÄs¡ˆ2?œSìïVÙ?ÔÙ½˜sÌ?û¹‹ô·Å?åoôým~‰?Ä~›B!t?ǀ®Ë¸ƒ?®o›ùƒ)º?ÒÉx¸@?´Üj›÷;?á•—ñ¿?µ¬}q\ô?¯?ÀURá? bTÓ©ÑC?à(ÇL¸Èç?¾ú£äe?ÛÆy[¶Š?¼ âVT~MIXED3FGL J2039.6-5618@uS²þÅm]ÀB"Ùý6÷äÀ8ʇkŸ‹À;O3·½q?úfý4Ñ@Y…kE-?û-x¦¯×Ÿ¿ÑӂMø†d¿ÝÝ'ãɾz¿ãˆã˜/% ¿í×)5óUNASNone?kG™.R?ù²o9¯à?îÎË™Y-? ùO	ô
?•»U,ât?•*®ô,‰·?''ôÐß?©yDB,ÓÑ?én¨UãÑ?ÆzP(6ï?Çó (i€¢?Ä\LòYµ?°¼¨tM?žu$.;/?ê]Rî†Ó;?¬eoùëœy?¼YJãÂÌ]?¦{™>ã'?¨œðõ¢¹;?•ÄÏæ"Wp?èá9û=<e?²åϘ:;>?ÆSÛÔýrÝ?°Í}}?'?—ÿWý¾?¢TAd©?îfÆ|6îe?«+{€jMÆ?›'ØÔE{°?›;Û^œ(Ñ? þð'?©ü¾i*&?ê#{4 :?Ã)¥J§Ãÿ?Ã2Ž4X½?½Ô1îÃ?ÉBÿ{ô?¯ü7L8µ?ækÛKÉ5?²Zʯn˘?º#	&f¾r?¢àéi?ºã9
b¯x?œKf¡BÜÿ?ègæ¶$a+?«7:v?ï§?ÀîÈ¢=#™?¤Éc]w PSR3FGL J2041.1+4736@U…Ó™o¨/@±€%TM_À8+Yª–AÀ:ÇvË8x?ûöžšŠZa@…4"@ÔŸgd¿×bYäfü¿äÒø/§Ÿ¿éN9¥Ni׿ê(±Žû'vUNASNone?µ
"©âë\?°ˆ1)}-Ñ?èWX@€E,?ÄÍûFÃïë?ÄÔ©²bá?¿•žÙ?«Œ¤÷BW™?µ0òÌ+?ß ×Ì&¬?Ɵ¼9gæÕ?Ýn^ˆÝšá?Ç
ÈRa?ÍTcyÌõ'?²iCåé²?à%ê(
?¹+(Ó,™?Ñ)'oÜ[á?³±¾fs´?µU±gŠ‹†?žÆ^®Þ?〳®3?¶Ÿ—>k«?Ó©,I4&x?³$t9[íò?ÎXU÷®LÚ?ƾ«¨Ks?å=Šz b¿?É&Ä7Ûl*?¹c<CÓ?±ýªÂw8?Ã$çœmÅ?ÃU•WYqû?à™®xŠ?ÃG/cÒ¦?ÖfXÓÅ~>?…7#¥?Ýõ¤-,š#?¶OC÷v{?֕›{N³u?³¥C(‹L?Æ逯	dÐ?¬(€bø?ÄÁ¿ä˜,?¢
­)?ã±>FÀ6o?«ì0:;'f?Í*E%Ž?£8SѵÖMIXED3FGL J2042.4+4209@T{ªOÊB¯¿²;X6LîÀ86‹ò)ôÀ:UÊ! áø?ú)Œì7 S@GØ4ß۝?þíâ¦Ó¾Ù¿Û¦IŽ‹Á¿èq®0Ý÷¿ã¡ÄZ"Ó0¿éãP÷,rUNASNone?¦7 ¸ï5³?¢eYû7Þ?ÕÜîØÑñ?Í«– Š±?ã®æÍ©ì?Î2oÒ9¸?~ââ›:¸t?â,¾ ¢è?όKalt?¼øƪÈ)?çß'bš~ò?¾È"!Qð?Ä
Žm?ª "&×Ê?Ñ~•Ç·Ë?²ºq›ò»ÿ?â=Q•ÛY?´"Xu?¥»?¹')9Ô?ªŠ—5JÁn?Î-ï²*	>?¸æÂÐ^Lž?åDCniÀ
?»«Øû1?¸Ñb[/t¹?ºZO0-´?àgðQX°?Î}6ïLËØ?Øý›ˆÿdò?ËɬåWU?"æû¿W?¤=°ïþ?ÔÒÐ;0•?».+ùÐ]?ä÷`ˆ·?Ào‡À[ØÌ?Ӆ‰QwìÌ?´Vâ"ÿ?ÏäGla?¯&>Æâè?Üðfä]?´('Óÿ1~?À©È£?¬CÙÌ-?Ù¢¸'ÇÝ?³ç`‡?ÞQc`ïÑ?µ­#-_MIXED3FGL J2043.1+4350@TÕßeUÅ?ëﵩ-‹À8"Íui8©À:· ×æÜC?ùƔ·1¯û@wOz;°Z@ªWk÷ ¿Ü7âȕ8?¿í§"€"¿Ø–§XÁYž¿î"i$ösSUNASNone?«:1D¿¤P?­ô¥¸C¥]?ÛT÷]ïõF?Ͼ͋¹‡?à¡á<N™?Л{#ÀW&?‹uô܇ì"?Ÿ{,ßrq?×ýyüÁK?šâ_í6¶?ã"k¤Á:?'
¤úB?̈I¶¾~½?®ÑÝJ õ?Øçzº¨ªP?³æµ€OҘ?ØÔ`iøR?¶&ˆñ¼×r?Ŭ
Ò)?³Cn¢qšÒ?Ԉ«¶¸Ês?ÅH"Âá«E?àP¦°V½?ÃpÞ9†´e?ºÿš»"?½ÊÙçt?Ú:åÿ£¹®?ÎÆ{ܼ¦[?ßـu—m?ВÎSsg?£ÈàÐh?³:˽]Á?ޑ,ò–#Ý?À!Üò	?ÞõЛRE6?½ ¡¤ï§Ý?Û©«ñ?´2ºA5ӗ?Ô	·f"
?±êƕ/?ÐwÌ <Á?°&ªm¢%÷?Ë©oé58?²
ë/²w?à"¡þ ?º_Cqï±~?Ñt·j™?´ÔNWÜçMIXED3FGL J2048.8+4436@U%+ÓÃa?át0‰4LjÀ8|@lÚÀ:à&¶ÁÉ@!­ÎYê­@"R£eö)?üîԞþ2u?Ç`MŸ½l¿çôò"䣿첻尿ïÿ" ¿mUNASNone?»^¡îI@³?·Ê¶"'%?ÞÁÂ%1›a?ÌÙÆ@§Ì?Úf•_<r?Ì#Ýø¾?P60Dƛ?g>Л"¨?âIõ·1;?Âí·#ÔVÀ?Û[Þþ\è?Âñ¢LÏ6?Ë.ð1Ŏ¯?²21ùžÓD?Ý9®!ôZ?¶r.€ýޖ?Õ.ÙŌDO?¶ V™1Š?š®Ó¨Þ"?kҊF­?êtÞp°?µók'n]ô?ĔR(5?´E]ßo–Û?ÁKõ?h?¿CEÅZ›?åÚyHÉÐø?ǑAhL'ö?ÇJ%ÉT?Áwü½ø•ö?pêÅÝ¥j?¬"äD)?äñÙÞÐ|Ò?¸f+üO?ÕØ¡*ÌK6?¸¾òP*?Ё8:jET?±ìmé‰éE?ÞÔi¢
º?´¼Nה×?Ъ^#ˆ¦?²"°y'?«x»Dè{û?"°§üS/?ê8s•gË?ªy3ÅAx?ÀA£aL(Ö?¥ßhþ·_PSR3FGL J2103.7-1113@BíÐ|"µÝÀA6)Çy¦µÀ9Í#¯1±À;¿VŸI?÷9`üÅ
@N¸Ê·H×?ñЉB37?ïÿxùsŸ¿×¨ùD5J¿â7îÕú⤿ì
Bùú­UNASNone?Ñ634ØW?Ç7¤¯Õβ?äÐae[à?Ëý"||°Þ?´¤(v³Á?¹yq%Ú?ÒuùeuêW?ÈàRxe?Ü&äzyª?Ë¡Zô?O?Ñcu´ü»A?ÁÆÛw›©%?ÒS½úÎ?ºÂÖÝO…?âå:œ*î?»RStqA?¿‡36IyW?§xWò³¥Ú?Ùjƌ°
?½P€òÐÜ?Û&£ó¯5?½_6ˇí?ÆÝííø?¸V@ïØlH?Úl2{°Ù?Ì`¬›²%?àg¶"?ÎÌ8«®?±Óøcâ$8?µó?I¹Sì?۔ÝL¡Ä5?ÉG÷>Õ·?Ù2RHÞQk?ÉrӉKåÿ?Æq ÒÚC?·Ùúõ?ݜk֒ÉF?·ÀT‡±??ÜÚ9/T4?·|ÆþkP?¶%kê‰Ì?£:hm?ãÂèn­¡}?´¯ôq»àë?Ó㯤Ò?±ÚÌ×Ãýš?²\mÎ(†K?¦Uàñ±ˆMIXED3FGL J2112.5-3044@-Ì`RP/ÀE9nÀY!À8¯¨tþ¯žÀ;N%@+i:@ABŽ@•ä¯—‡Ç?ñĐ£PҀ¿ºTqu§æ¨¿ÐSF"ã!M¿áG¡>Ô|¿ïÿù_|è3UNASNone?¦u¼RzM?·»áȓtj?ìÎÑ®]¡?ÄÊÆÿ­?¬çݦ?¼Ù¿ $´Q?–ÏìÚä5?±i~¸ô|	?é­ÀªLÇ?ÈiÈlQ:?ÆnÿºéS?įHçiJ
?¥Sfàä?–´»¿ß)?êÙéjš?®6úîí4×?¾‡'åU¸?ªôG ^¡ú?¬-lhÁ±ý?Ÿ2Ȅ\©K?élj	14´?¸µXÏRwÂ?ÁրÂT›/?´ÉY‹½å?¤I³ï"}k?´tžTƒ)?ìçMò[…?Å+N•íÆ?­A{ϝüD?À¸Î4£B1?£…ܾÖk¼?³âw÷æß{?êOÊ˔ò?Ç5Ë`]…9?Áß`ŊÉ?À(VÁèb?­RYüçù?ž®öGü`<?êo•"a#1?®¯ŒWä-í?½Ú&ß_Bþ?ª-º¹i3?¸b®¨¢à? Ùd†xÇ?êjËjç?¯™Uùr!z?·úþÔ¸?§;ÓÄ|‹PSR3FGL J2114.0+5239@WWn.±Ä3@ßT•Ð·À9,Òn¥ÐÀ;ÚPp[?öaÅõæ@)0¬›)?ô"rþ¥7?ïþ,0Á®¿çX/ŽZn¿ê\¼:û¡¿Ù­k+$ÏvUNASNone?ÞSm‡º@?Ï:(€
?°•ÆSD?²}ƒ©yRÖ?ÝÒe‹}ª®?ТSå¸ßŽ?Û¢ÁÀ"O?×ö²w>®o?´''Ø>¡Ð?¸xÍ#èE,?ß<™ÉjA½?ÕxR&"g¦?ämXóâ?´-!ZÊz?Ã%1nHCL?¨¤@Ý,û½?Ìe-è4v?²â
¨i?àBÎsê?Äǐ3$«Â?¿¯'¤=ó'?»ê€o"¥Ê?Ø
•ùÀºŠ?Åmð‹_'?ççax•é?ȐHaK?±/ƒÛ%Ý?³d!†›6¾?Èðà·T.o?Ç­=\Ï0L?å/ùÒ`×Ô?ÖTøt	V?°‡5w{Ð?¶Yݨ"…?Ñ~J΅^¤?Ó
£}Ú1 ?痎Á'v?°™¬´G}•?¿¡9÷Ñ?¦ë
îiÐ_?ÁÑ#?ª€õ%4³?çvšŸå?¸ó™Áá?º¥|Cûàê?¬6*¶dâ?ÄÕ+uϏö?µÑfS_èMIXED3FGL J2117.6+3725@T³ {5+À Œ$=Ìê)À9´ã¡ûhÀ;[«Åìû?÷º¢˜›Â¿@ImÖr=	?ÿÚ.ÌHî¿Å~Þ]ÕŽ¿å))'¿éˆWHÕö†¿ïÿÃ	ÌUNASNone?Öd`"´Õ?ÇTm­$i?צi÷óö?ÇíeU'¤O?Ñõ‹swW6?ÃÏûu¬ªm?–ÇÒl<ø?›!qŠsñ?åÃk{›y?ÃPçà4Ä¿?Ó««~?Ã{cx ?ÓÀ–ìÇ?´w€âàØ?য†Ôe?¶ÐÙubê?Ç%À½ä–\?©¼¼ºT%ü?¾Y
âuð6? ÿcÙyÃ?ç.òûH?²¬× ü"…?ÄkÀ²&?®"œ)oN½?â‡í½2P	?ɚä‰ú6µ?ÒNH~Z4:?Æbˆ.üÜy?ÁC¸'Wf?¸Y4?­¤á³O'y?¬Ž[ð8.?æd]͐—?¾ìíWözà?Ð@›vÃ?½'5Ù?ßøéai7¸?²³#ƒÕÇy?Ø/Þ}Vöd?±}ßV䩒?¿\à"ÿG?¢í°]…‹?Ò7†…2?¤ð>Û¡Àž?ãw ƒSl?«%Ó¡˜º£?»hã¡ÙÓ?¡¦²â¹õºMIXED3FGL J2125.8+5832@X¯iì,äe@Éú©u°À9'][û©YÀ;ˆ*…È?ö9B×@I@MãÂË ?øÉZí6yº?ÒÀÖc=Uæ¿çmõ*ÜD¿ë:¿»Óg¿ê¨»VO9UNASNone	?ã{
µÓ¿Ž?ÆRzHµ??Íð7¼k?Ã#¨H*‰?Ä#'lEðÇ?¾i	6"¨?ݐÁäfqy?Ñ¢Åý¥²­?Ê]©|CP?¢Ґ¹©¸?Õ@i]wæ}?Ì5+t¼¯?à"žšà@?·¬j'òç}?ÔÛ!K ²?´\ì؂xñ?Ã÷Bþ=™O?¨QLϖŸ¢?Ùü˜Ç·#?»sÍË-?ص©øýÙ?¿Di¸¹G?ʛz€Šæ	?º³/9Jñ¸?êAV²œÓh?¾…Îze»Š?ÂÿXV>Œ>?»à:ñK9î?ŸÚfð"]?ßçñé?çø'F(?Ð	S7¬áí?¾Kҕ¨b#?½Ð¡FûÖ¿?ÄÊ6dÀôÒ?Ã΀IDG?æÏ>Ziê?±œ´sÖ	¹?É"¦óõ/Â?®>™¾ÅÇ?·@¿DX\~?¡ºv¿íÜ?åZnçFÿ!?²&5
œÙg?Ðgˆû;Ë?¬ŽèBwˆs?µ"ꢶþÎ?¥Íáû¬5AGN3FGL J2133.0-6433@t‹Ò½<6ÀD¢VÿÁßÀ:@ËLš†À<	—@G?ùþð`z¿@B°'¿7Ž?à~ð~‹Sä¿á'òWBT¿Ã4Ì}‹¿é@¢¶½…¡¿ìiµþK—PUNASNone?¶ð§Áê4€?»Ùýº£?èm+{r«Þ?Î3  °?ÂÒþ0-UŠ?Éq'¹Ç%]?ÔN7`iw=?ÐìSûª°Ã?Ü/^x—|š?ÑBÉC*w"?ÏÔMþR?Áe¾ö ZÔ?ÇÂõf&®?¯œTf߈?å4ð	'ÐÓ?´Û_m\?ÃiJsŽ˜?­X·Ë4¦Ž?ÙÐöøš[?ÄÛ>w‰à?ß>½¢YÔ?ÆW³3°?¼c)'
,†?¸±qª ×9?°¨Aú*?¹†lÕÚ?èu£¦kl¾?Ñ)£E¿Ó?ÅÕ1Ä·ï4?Îw¡¹ÆN?ã)êX½ #?Óé'ª?Ò1ù¾-³Ô?ÑÁP»&?½èÆA\/›?¶#Î7ò9ã?ÓNq°¥Š?¶Êá&fÊ?âª&ðNæ?¸a²ta©?½u¹'¦?§;Üê]?ä^]¶òùe?¾N'ÆQï?ÔrðO*W?»Ð¯M"G?¦'¢ÅãD?¤Ä³/º$KMIXED3FGL J2206.5+6451@Z¡ï^Èt@'W«¸€À92FÀ:ü¹kÆøw?üÁ"\Ð@ef»ü@…újꯌ¿Ïøå!µåÞ¿çғâº8º¿êŒœ",r¿ïÿ"Ó¿¸ÆUNASNone?¤YØ««©Œ?£X%­yûc?á´sÛ?Ðc"Î(—y?Ú†/|'?ÐTSípŽç?"çم¥?£$αøaÛ?é.ÕNŒ¼"?Âô`;ÌVR?ÊüSøû?Â~kž"?ÌËj=Ð|?¯îŽë07?ÜÏڀ¿ƒ?µÇ|
Q(:?ÔÊËñX??¶Ù«ˆë‡´?˜l"rX¨‡?‹*Ü{g?êª?†J(å?±ÏBöY?
?ÂI}™Ö!Ø?¯"–?/u?©²è»Žã'?­–ôK1zÎ?߉½I¤±?Ð'9x.?Ý?åÎ{xœ?ÐI	ŸÍ –?—@©Œ'$?£î@pû™(?éG<\0d?½HÚÎÒ?Çúù_@Ç	?¼[$"6"?Ô?)`¡€n?²¾¥â¬?Û´[ÂœH?±Ìä–4bÈ?ÐzÝ@ãJ?²Ol=A´=?§
r‡¢oX?'¬°™®?ëLò»ÈC?¦Hù<C1–?º5ß,m>? ²o½ùPSR3FGL J2212.5+0703@Q/‹«`kÀCHP½‡µlÀ9nv½ÌÀ;™FéÉ\Ö?öÙù΍—-@4~…l?ûHÙÉà^¿Ö$;"Ì"¿á*øú¹U¿ä7û"i¿ïÿåFúUNASNone?Ò±'ÓsHç?Èt1¸Yd?ã»ýϧC?Ìšù.ïF?·Z5€Ö?µô¨}Ê÷"?Îâxۈý?Æþà'žÊþ?ß]ƒú:?Ì%Tßf"?Ñb‹¾˜4G?¿æ)6§~V?ÐÐD~½¨Ë?·µœ‡@A?ãž
å¤g±?¹žv·½'?¿Î~×æH?¤­f;Yƒ?Ú%˜ª?¶Nȉøåû?ځp?º(sÒ	͉?ƳâÃâ ý?²ø…Kÿ"?áu¦Õí1ò?Î$Q ˆ6?ٝwÑ#‡?Îíæwî¤
?«¹Ô˒£?ª!€3×?Õû«nЏœ?ÊRh °í§?ޓ5À÷©?ʹAÑAâµ?Æâ=¢Lñu?³0D?,ã#?àn?;‡É?³vJñ&/?ٝYÒ¯9ê?²sWàۅI?¶žÜtkª?Ÿ(ËÑ$Jb?ã(O]	?®îVùûß?Ôld¶Ò©I?®¤¤k'ü?±Õ*©Ì'?ž³LŒåEMIXED3FGL J2221.6+6507@[¿Ž`€@ÂQã!¢èÀ9gJöžWnÀ;ç½?ùû÷²©‹@M;G(Þ@…xì?Âyð‹1»©¿æb©\h¿ïÝÂ凮¿ïGKI½ÂUNASNone?Ó00áì'?̇ݙùÐ?㋎ó±æ?Í7á,]à?¶âÄߚ9:?·…ßq?̇÷5¬	?È#šH{?ÛTÖŠ×"?Èñ;+?Ög§Çqª?ȸóõcM?ÓÐ'ƨ?²áNœT»Â?Þ>Ëf?´}†ìjbO?Ëâ?Ê4/÷?°:yð‡—?½VnùªH?¬§•ÑP#¶?å­Âu=?ÁK_Ãè€?ʝìœmUæ?º•*–xõ?Ø·6‹ê?Ђ%vSÃ?âC¦²J¯@?ÐUvÿ檙?¥Q[.¨H¯?±ÈÇaVpË?Ü*ÚZe7?ÐKÝ¥"?ÔÇl›^À«?ÆsAsÆSê?Î<Ñgò¿?Ã26ÏÜ?Ýc¸¬?´ý3ž/Xó?؞ ƒ\…+?³÷ã!?ÃüˆÍ՜?©âDC«ðA?Ð,Ç¥+Ú5?°Í`;¯!¤?ãubòWe?µ#s&ÝM?Ã4›)Þî?§çBûÅa2MIXED3FGL J2221.7+6318@ZÁeUÅ.s@›¡±–À9(‡%ùŽÍÀ;&'d@ò?þQH,>¢R@
;ÏWì{?ü2ßã«¿Õ4o)>ÎÙ¿ç¡äÞ³Ìm¿êüÇ`sª"¿ç"îrA™†UNASNone?Èw3h7Kò?ÁÒ>S£Q?áLJWfˆ?Î}ŽÜp?Ñ ×<"¬9?ÈÝ^jnˆÊ?»¡Ö)û?Å»'ÆIX—?ڃï
0ÒÓ?Ê
7¸ ga?ޛ¨€Dçn?ÊHÜ}Cø}?ۅPÐÃ<?µXlüb=?Òòž»õí‹?³CŒÕùl?шu/ø?µª¶'Ñ$?º>"ª
nÞ?°Z6VÞq?äE'ðg'?Æ¡)óeà&?Ðå4õL•&?Á°ŠÄ6¿?Âý'ùð¤÷?Â=ôž3B‰?çƒ*|€Y,?ɞ¼8ù5?½ëˆ,go®?¼ƒ#WëEÖ?җà ç.?ÒèBm‰,?×çéÉ1â¦?ÊÚ䙁 ?Հ6ù|ê?È\pl,V©?Ývî;æ?¸ÅsX…Œ?ÔM/‰Þw?´æÔrÎù?ÌxË5ŒÄ?³–ÿªIß?ìùÄb×!?¯Üykl«?æãYØË®?¹§x?ÀŞÛ!ú&?¬'hU¨ÙMIXED3FGL J2233.1+6542@[UîËûµ@>Û<ÒfÀ8ɸKgÝÀ;ØWDŠt?ú³
-ºù;@¯}W´@uàŽ ¿á"ŸÇ±¿æ±.–kfֿ놥¥Z[Û¿îljˊfUNASNone?±zP#êüõ?®P?T
·?ëEè¹ß­?¾$×óÿ?¶#€•j¨?µQÙÞÐ|Ò?ªŒ'Aˆõ?´êcù‰?åA~Áë·
?ÈmJ#mK?Ò+pT.‰?ÇëÊë¥"?Ö«½A®9þ?²Ú%Ťt?ÜÒbDæz?´>_ÿG‡ú?ÉÀòׁ?¬Trø3ò?²`ŒXy¤î?œóîBËÿ?èDqœØñÒ?´?ndÖ?Žó`_fB?¯ðù,ö.û?Äl+}Ã`y?ÀQÓ$ˆS)?é"Éîöî3?Â7§l¿?¬"³ó6á?¨g'rþl?Àí¤S_?¼¾DÅhÅ?ãÑÃçs1?¦˜°?ÏËLœ&ß?Áí‹Mt›?áïÔí5V?´™# ­¯Ý?ÔòKý."h?±ÙgËwT?À¨±îÙ?¥YÖôd?Å75Šs?¢Þ
YRà?揢Bh8?«®©È§(l?ÀŠAhfW? K\ø8hMIXED3FGL J2237.9+6320@[&E^®â@öj}L[ùÀ9Z¼ËÍÉLÀ;S:ঞ?÷¼©ÑË\@ T´àó@ü«¶Q¶+¿Ë1Š$Z¿¿ìˆÐí*¿äÉiý
¿ì¦
ÆŪLUNASNone?À[búÿ˜°?·¹×â—d?áCpdŽl?ɚ^n(_?ÕÇÇ¢É÷Ž?É ©Kpõ?·ŒŸr¤÷Á?¼ÅÍ÷f À?ÛG›_—j??Äö}'.:r?ÞÕ<ÄÎp?Æàž¾?×4({Ÿ3?±O»á	s0?ÝGËÐ<\Á?±öÁ{«Š?Ç6?§Q…>#ïL?̟'ú:—?°¥÷uñ3?ßû«]¢ƒ´?¿¡cè¹V?Ñ´‹%@4?´«É»k­?ÎGØòÇ?Áý3«(7?á1JÙÔ-z?Ɲ)³¤ÿ÷?Ìòû¦3P?ÂUÈm†Z?Ð&i	‡$?ÉvƒâD¥™?ÙCx£ˆco?Â͵ÕåO?֖@nn?Äž^`™¯?áH×û‡¨ß?²y=¯h+ñ?ÖX©& ób?±$RÍZÐ×?¼V›‹>ë? ¶j*~ó?×.]ú×è?­¸Õ¼?à‰Ø¦Ÿ¼s?±Ù@ÌVß?¾÷ÂâƼÆ?œÒÚÌPAMIXED3FGL J2310.1-0557@Qlvò¥¤jÀLø(¡ß¹9À:b8š{@éÀ<5[½•ø?úØ1rìí@Pž¯®?«ɔ•)?ï¢Z´ñ'º¿©‰ì	!¿åèg™±`¿ïÿyOw6˜UNASNone?ÓILHdzÍ?ÔúNìˆe%?äŚþI
?Õ£ECè?©[ü™ÝÐð?ºhU‡úh?Ês Þò¿%?ÎÔbI4?â¼\P6³?ÐߣÅ}´G?ʛmà"f?‰ÇcEj?¼	U-Ý?¬<ñ?èùl+æý?´®œ"§›?¿w+Is«7?ªpŽ$É͏?Ø0Í]"Í?È]¢>ü?àÙª¯|Á?ÉÆbZ=8E?¸ouUñ??¹°'w™ó?ύ}£ç?Ó?:×±/?æY&a‹?Ô_=äMX4?«œ9"v•à?ÀÜsJœÓ­?ÕûMä9zö?ѱº\ݦ?à	ùžÅ†?ÑÍGñÜ%Û?Ãá}¾œ³U?¹S-§®'?ɟ;Ìp?´>V?æEs|úú?·K·\Ö£?º–1§Gþ?§"††<Ë?ä[³"ý*?Á·쵺%?ÕWG²Jk?ÀJþ$¢eŠ?¤RùÁ?©øóù	âDMIXED3FGL J2353.3+6639@]M©?)
»@½?é$À9)ölÙG/À;O{ƒ.J?þCaƒ‡4@
J^Èã3?þi™aܔ?ÒéQ؄*¿èñôgN }¿ì€zŸê|Ç¿í›>ŠTWUNASNone	?¤È%wwŸŽ?£ö¯RÌ'L?èú'ðŠÂ?ÅöŸuÒ?Æãêá	ðš?ÀØ2?èÃÀå?™YŒeÿn?çf"mW
B?ÄÅ©	¤?Ы3Þ1¶?Ä^ªZ\?Íh¡´Æ×?¯8"®œ.K?á	,~ã?´NŲg í?Îr«ÕA¡œ?±Â[M?™‰ïÈ`"?@ûe‡?ë¼Ñ¦•q?²á*'ِ_?»·.Í?ZÖ?°´L¦¶]?Œñ£|䅐?"\T7çWP?íœóÇ0q?µâýB æô?®ôZ±+¥ƒ?²¼*jY1—?›åyë3¬?¥‹o]¦'?çH§Ìë´!?¿"t&–Ë?Ï`±Ž¶oF?¾ÅÝHÖ?Îv¿ò@F9?°¹ù–?á3ÑMåæú?³}vžþïp?̹úÖ(ß?°¾ªy™?°´ùs–G!?˜×$||¡h?ëKDVÇ?¨r'/m÷l?´ðãÕÃd›? õi'þ•~PSR3FGL J0937.7+5008@dëÿ´€¦@Gbž À:' €©ÌÀ;ömÏç3€À!͋¹‡ @8e>É…@äÀ^g¿â¯îyèÓ¿ç'Ã&l¨¿åîÏÜÕ60¿à¡xhÐAGNfsrq?îV¼sÒúR?¸¡'kI'*?5"_þí©?Eµ×LLä?ªiô¤R¹?¸¤Ü)Š]ª?ÌC:?­ è2?"æç4"ø™?¡÷i? 4?•HÿFsa4?£0íïÃX?íY<5‡Ä?šìÝ"R?7³Ù2w&?ŽÍü¤`/?«ËRTYË-?"¶Zfö%®?ïܤ5©Û?Œj7é>#ùs>D‹¼Ì?q­ä'¶F?Œj
ÙÀ"?íEˆKO?ÂÚCýI±?%tžæƒÀn?1®Œsó[Š?µÉ³ÏV?ÂÛm›Ü6o?ï"Ó&X.j?'¼ÐâMk?xn–1—i?…Ý'ZY_9?}§Ö¯_åª?"_ú±uz?îg9åKk0?˜|Osë-?˜%Ú0íƈ?'ÛÌ¥ý®?šòé,"v?û&'	3M?ïÿ–~°•?'Œã¥¼íÉ=Ë)ÿÝuñ=æî_Ÿä
?
`Z $e?'ŒãZø¡dAGN3FGL J1031.0+7440@`ǗͅY@CšÀ ýÀ:&sÔ
2îÀ;´¦ÏB.À!͋¹‡ @M†ÇÚʑ@,"ß}ÿ_¿ÎY 
ý¿ç¥b•ÿä°¿Ü[z"0t¿äSr€'TAGNbcu?ï¹Û¨2?™¤ •v?CTÛï?`R¤¯Ð§H?€SÕ%r¥?™'rÑÁ~?î®ÅÁt¹?­•Üž¥
?•‡9ŸÒÑ?¢.£›>ú?•"À©Î?£M€Jÿ¤?í¥«'œŸU?—–+™ï|f?šˆüυ?‹\Ì侓Ì?¨`Ém—"#?',|ØB‹?ïéw]¸Ÿ?'2·@›">jò!ö>;åã^La?fˆ¡™T9½?'2¶øƒk¦?ï×mëüù÷?'Hv?~C?*€|¡täË?6í+_L?su<Z#b?'De]óhQ?ï%T)^?"X漆/?y²³Ÿ00?ˆˆæ8ƪ{?~»c"ü¸?‡M6'"?îÚÂAi¾?_èî?'üã†pÉ¡?ŠÇÎ\Û'w?'Á"-òb¦?ƒ~h9Ê?ïÿ°³ÖJ"?v˜RÓ/=Ìk°Ü]»=å@úcoQ|?ÓÞZ‡>?v—\íÃAGN3FGL J1159.6-0723@q'Êßø"¼@J¢€dÀ9Ҙ×ÒºMÀ;¢Òhî#À!͋¹‡ @x†ä'@Ôɀ'±¿æQ:›:G¿Ør‰ñ¹t¿æð±$´|¿¯ƒ-–mžAGNbcu?ïiã)õ5»?¢yžF«?l™õö?€¼ÒXzß?Ž`îxY¸?¢&Xñ£?îz1æ?®î›"·ŽB?˜GK‰b?£ä6i×0¿?–BIsÏ?£–í´ý6ó?ìhÑðÎâ?¢÷Uª'?¥sV²ëÚl?'ü¦ëLûÂ?±ÿÅ=ä»?[Ž~nT?ïð
Ÿƒq?~¡v«*­'>±îÖ鋢>2±vC?_äÀ;sco?~¡v"iH?ïiŽjw©@?«vŒ}–¦?bÇNr¦©?z3£]J-€?uHèXÕ?«C nı?ïˆC39?'åâmÍ?{ß±òO?‡õM †?þ´et¼Q?…³Ž_/º?îl͹ð…?•µÝŠÏ?›aÁÎÝlY?'<\
܇?—‡	…K?†Lý¥*óÿ?ïÿýf?":PkEÖ=Án81ù> =؁X E­>þ!A¨ñ?"9ôðŽAGN3FGL J1832.4-5659@u#–Óõ¶À4¯ÿ6¬dÀ9>ô×­Ñ_À;–Ë1ÂëÀ!͋¹‡ @´:¹ºKk@'¾Ÿã_¶¿é!á+ ±¿Ù
¨4¼ö¿è­·ŸOLU¿â.e-"ÅIAGNbll?펝kzV?¼è¿S‰â9?‹÷"­å† ?Ð\/s
¨?°$àÀ
?¼lόÔ=?ìq>!´ìÂ?¾Y¶Ìý–'?¤c¶³ï?°Þv1G'?²sÝb}?õ?²­òÆ&i?êUèŒÆÍY?¨³D×É µ?±¨&Ö&¿g?šÓT"Œ¼?»¨"Á Ò?£"²° ?ïÂÝ×zêq?˜w6™>$/r–ݦ>CRº3Š¶™?~'Â	dU?˜w/{ª?í˜lÛ z3?ÄÙ¾‡?˜²9'a°¹?½°9ÿ$?ª yWèq?¾+´±´)?îîÌÐÂi‹?¬y-âhà?Šl<¡îh?œ$Ò2Âhþ?•/Ä:mi?£c}á~Ëè?í^ˆ'qmg?œÃ4•»?¥ëÀ/ñº?–?ÝµÅ?¤,qI›Þ?'9Âüį?ïÿV?:L)½vZ=Õ0÷×°»=ð× "ÊŠ?U-'µÐ?:L)~Êz~AGN3FGL J2358.3-2853@5H€_5ð}ÀSŠ« ,ZÒÀ:GpJ붝À;õxZ"±À!͋¹‡ @žIaÈÈ@OãÀYK÷¿ßÐ¥æ?JÕ¿ê®tŒóe¿ÊTLªË¿ïÿ'£+ÓAGNbcu?ïpÁçŸ?¡Òrɹ+Œ?Ft°Ôè/ð?a:]Žz?‹<""xd?¡Ì°#G"–?8'†?±²x$)t?•˜Yn)€?§ïQòf}?™Uƒ'°Ç'?¦ê9h	ô?ëxR'|¢q?£U«ë>$?±h¶çäÿi?š:öXÞÔ¼?²Ô´'~?šmÑúÈ?ïì;<—
?€bd"£<>	º˜Ñ_­U>0XÅIõ?cÄÃ@3D?€bZEÏK?ï'^N6f;?¦®~H©hÏ?AýÛº
õ?P­|3ô£?ŽHŽ¶§÷t?¦°eÉ>•?ïl6¯"'®?¡{Ž³	ø¿?¶ÇP3?'ÿup¹^X?…µ?èM?–äglLŽ·?ììDiïæ`?ŸU•¸þ(?¯Éöiå]?šÓ¾/Zs…?¢ïi»Í¤?}Z4.#ã?ïÿ¼žVlÉ?. 'ƒvÊ=¼¼*†àQ9=Ù=4d¤€?Øreiâ5?.Ÿ¼3AGN3FGL J0534.5+2201i@g´ßݵÀö@8ªAÀ5¨†¡oPñÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ú=p¡'Øa¿Ó×o9ìh¿Ù3Ší•€l¿ÍÉB˜o¼À¿ÍЁ~+^OTHERPWN?è?0´?Ω°ÑL@ÿ?·–HŒ
å·?ÂHD<oó?Ã8ZJ›§?ǘ,F¯çº?¹hhè)}0?ÍGà¿Gþò?ão8†â»?Ҟ¶ê'&?ÒÇÙTçÛ=?Ð:!
Þø–?ç ¬'¼þ?¯áí蝰!?¶Ä©ÏEÏ?£ÓuâŸ
á?ÈlfIyà?¬§bŸa¤4·b°«ìß©5¯8|´?ÃD¡*î§N?ÖyPÅ%Ÿ³?ë.×µDV,?ÖyPÅ%Ÿ³?çý¹Ir?ÑfX€?µ·Võ@o˜?ïȲ-[¥?Å-p=L3,?Ìù!šël?±4ÀA6?ÇúrŠ¿"´?å{Ï@af?ÎÓó0[?л1Øê¥?È«0-LòÕ?æº-t³?²û—∖?À ƒkÚÅ?«ù½Ü?ÇUĞô?¬ö-Ëî•4·¼
õÅ>56¿Å05û?²¬˜T5?Ш%Îp¼?í¿*múy?Ш%Îp¼MIXED3FGL J0833.1-4511e@puR}ÔAÀØðߦ™1À6!vu¨"ÉÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@G̀&¿äqªé3q¿æe¥åþ™¿äqªí~óü¿ä§ÍP¢§,OTHERPWN?Þ¢­­*x­?ҟ‡ìëG¯?°$_a"a?½Ç¬ô·™×?ÝT:'˜»›?ÒaÄaˆ?¿c,Ë2x?ÐS3[@˜?äL>¤wæc?Ò®z›ko©?Ïo˜Í8?ÌiúZ#·ë?ä`ô=»?°‡‡a,ø?½$'?¤8>ÛH?Ïõ4ú!ˆ€?­ÑêMN-4ÐÕ^®|%—5 ™ÉU*?¤º´ò:›?Ö2xXr?ëVÑRÃqY?Ö2xXr?ãNX¯³P?ÓzÉßä?²JÞ¨²à>?Àí@RÞý¯?ÔÐ
¤Xdp?ÒUODXA?´® âš0Ç?Ë1ö®XÕ?æ3'™Åä?Ï߈³±?ÌܑGÝ܌?ƽd~HŸ?ä:àYO/?²¦zm»a™?Ö*æÕÙÞ?¬@†öc'?Ì镟'è?­°£³dK"4Éý
Ûxû\50ìÅFæ0?±lizÎðl?π5HÐî?íÒrÐÏ]B?π5HÐîMIXED3FGL J1514.0-5915e@tQ¿zÔ²¿ôWõÀjÀ7Ï{-ÇýÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ù$5½À¿Ñn£ Öå¿×!ƒït~¿Ñn¶t¤J¿Ð…[/aӖOTHERPWN?äÚóÖüÑ?ÑÛhéDôô?¨ZSÕâm?Ɋ3ªÒQ?Í9ÜÎ*N?Ìwµiêæz?À-ąÜ­?ÐLlÑ©?ä8!Pÿï?Ò-û¹I?͝Zõ«#–?Ê¥NŒ2±?挟tâ?°!ñX§žÛ?¶œ8Š¼?£fÜbSù?ÌC±>ÀžÛ?­¢þ¢PÛ4Ä«Ò¥*Ç55d°eœð?ÀrÝ~\
?֕^û§Åp?ëãH hý?֕^û§Åp?äóSU¬H¸?ÒÊC‰ÜQ?À<E9´Æ`?Èg1zÔåþ?ËömošÂ?ϧ3Øl	¶?¶'&!W?Ì>ÐuMßÝ?杹ün.?ÎȐ¹1uª?ÊJá…kE?Äs]/[k?ævmK?²'ú•0I?À[0nCÛ?«†¸­
;?Åʍ޶•d?¬˜†˜6Í4Éc¡ÐSÝ5Ÿª¹2¤¡?²3æB†æ£?ЇŸàÊI?í¹ƒ7"¦L?ЇŸàÊIMIXED3FGL J2021.0+4031e@Sp¿ñ7@'˜à66À92šs´-Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?øzá? ~æ¿Ð&
ŒT¸¿Õ¨xöræ¿Ð&
±Õ‹É¿¾pç&räOTHERSNR?ê®ó.Ðé?Éx}²'º?²³M2@w?ÁPq´šžI?·ÕXˆÛ›?ÁÄO°lné?¶§x%lg?ËbׅãYV?á雈˜Pª?ÓÃè³ÄN?ւêÍáR?Ѷ9°ÙY×?éŠ^ÿ¥ù5?«¶ÂÞÝ&©?¶ÀÍgÌ?¥õÞw›Í8?¼ìEBΏ?¥BåÕµ¾4ÙoF±´)5)‹"½(°?ùÙc5Á?Ö´r[oÆ?뉻ç2?Ö´r[oÆ?êL¤?Ý2?ÎÚm^(?±¨í‡rõ?ÁÈ+aqxØ?¾
ñíåî~?ȜY"â?®ŸÎ·¿'©?Ɣµ0pW£?ãOYººO?Ð;*¤Œä?ՍR´ú¬?ÌÅI«ƒ@?鱯yø?±6¤í¢¿º?À]Æ(\¯G?®+Y7ç"?±¶÷Þªb?¡ÁãÜ%2Ô4å$tò{­53A‡º\/?²x;¬d³š?Ð7±ÿäH·?í°øŠ¸!¼?Ð7±ÿäH·MIXED3FGL J2028.6+4110e@Sæy€žQ?öVŽà3·À5$‹
Š}Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@ff_°iÀ¿á¸•Ý0r¿ãêáF›3¼¿Ê²ôQ©ž}¿ãÊ­" ®¡OTHERSFR?×u®?¹?ÒÚô\!­¿?¦·Þ,s?¹'.
<_{?âÙ·Ÿq¨l?Ó%l•Cbo?·¨Mùsy?Ì,¯Ð+•Ê?áïÚŠÅI?ÓT	Âvˆ?Ö68`Đé?ћ{4îc?åp¥'¨v½?°Þ¶êr?·''ñM?¢¡‰gH%?Î|\Ÿ	½e?® ü݈G<4ÅÞç§8ï&5'>
cIÝ?Âæz?X§Ù?ÖP0¯uN?ëFap)Ö
?ÖP0¯uN?Û±Åw¿?ÔtßA)Ò?¬(,¯`€H?¿Ú±oË¥?àdš±*L?ԛæ¸'Ɛ?®ÅI±àô]?ÆÅ?¶:?ãV4·?Ð<Ðø¢àâ?Õ{8—Ãx?Ì´dUêî ?äàt­Y‰?²	ݦ8F?Á9ђ¯D§?ª'µ³We*?ËD[·êE6?¬ÜÑf_fŠ4'nwçr;5[4JßP"?±·Ö/´éû?ÏÁ0Ÿ¸ #?íÉ9û¤Q?ÏÁ0Ÿ¸ #MIXED3FGL J1513.9-5908@t#àz(»¿ò—™:À7Ó%ô†O:À9ø˜˜—;À!͋¹‡ @d<˜â'@óƒÀig"¿ìÆ¿u)¿ìž=e^¿áÃn/Ĥñ¿ÒºTûPSRPSR?™þ'g‡Rä?ªI̟ýÍ%?š
Œ{R?´¡ÏN?î_·´?º™²-º"{?ë`",Ó{?È'€?¡¤qè9_©?°Ì"Oˆèí?¾ÒÂçèÿU?Ä"…)äÅ?Á9'¼»i?¨ç'½4Üß?Ëڅ –'?±eĔ&åˆ?ä»ȱVœ?´Áb?ïø—í¥"?h:³
4 =Æ\/ì
Ú.=ì…f."}Î?Oñ Ü¿Y›?h:³­\"?"äb"?¤!sö¥l?žŒòW…á?µÜy‹‹?î»xKÁ™?·ìËCۃ?ît¸?»Æ"?µÊ4ŒN­b?…üò^ ­?"—_,àþ?£5?k¿…€?³@öÁóö?Ő
ÌÚ?¬îtë£ø?Í- ½˜Z?°Éòû"<f?ãP´]Bž?³Ž0õ_Jæ?ïÿß7×#?´ðK¡†B=uê5i!˜C=ŽxðƒE±P>ðd'Hžÿ?´ðHýü	MIXED3FGL J0121.8-3917@qU{à~íÀSË¿ñò÷À:¾8äMÀ;ÿÍ2MZ&À!͋¹‡ @èw9@?üÊb&%Ú?ïôöŽ®¿á°ãôAí¿âO²vE'¿ã2ã#žUNASNone?ïßhҖ);?""µã*u?6'ËÝòâ?QÛÏÈú`&?mÒ4ʾ›?"0Á'H?ì嬕}]×?½£Åµ‰í³?¤'[ʽ9B?±Üô9?­}Úß$·F?°2:Åæ¹?í`'År™?›±
4¹­?¡ØwGV£?×±'5ì$?®©\aÍ?•[PKth?ï­¬¿¢S
?Ÿ|rrÞ>ûxiþª>=YTQ'?""ÏÈd99?Ÿ|gǞì?ïѤd"â?"kG¿§ã?'W£8¢¬?4ñc§C~ù?vqt"‡ÉÃ?"iAxu{?ïkÁš½?¥ŠVîiΧ?‰5ƒo‹©?šÍSaOEû?7ÆÐIÝ?"p²
Láº?î˜\qY}?'på&}Ç?•î_ɳ ?Œ²Á(–Ü'?—àƒ{³<?‡wö"m÷?ïÿßh÷?6*zìŸñ=ΈØ(\=äwˆç/¢´?D
cõD5?6*z¾q þAGN3FGL J1655.1-3954@u',à2Û@ÿ8x[0À:fÿš6À;â1¸ß°À!͋¹‡ @;,‡óSõ?úàåáâ"?ìºvçpš¥¿çIÕ·¿ÔuÌX2¿ã'?™UNASNone?í9ºù]?ÂÓÛ¥¾Ò?PhÏ@RR?p;ø§7¼?µð"ù–²É?ÂÖ½À¯!?é©Ø½,,?ÌR'
j2	?«.Çÿ²|?¸',ÁÇ8£?Œë
z'R?Å!	ù0¶Š?çlyW|5'?²ñfÂÔ;Ü?°Æ®ùÈÆg? ±¼|ÒÌ\?ÉêÃ$Ná1?°÷pà‹ó?ï³gïä?›õ€¬*l>2%á0ú2>M‹&7K¯?ƒ&k¡M?›õ€'e?íBæÖ–T?ÄþýÝ¢?Ll²z!÷?kþÞm9ø?µ¯ñ-îês?Äý˜=?î$þôV~?¸µÄZëçx?°S©ñþ?£ÃŒõ?¥Wç.¹+#?³ƒL}ã?ì:–ƒ±ó$?¥
°>c?£ï!ӒÎI?–j·
8?´3ºúÌÁ8?¡t•<ãl>?ïþöIë'ù?7«¦,pôV=⳶Fî=ø¿ÆGüj? ›_4ð¥ ?7«¥¾}tïAGN

==> SOM_VIZIER/3FGL_prob_catalog_3classes_SMOTE <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  312 / width of table in bytes                        NAXIS2  =                 3034 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   40 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\SMOTE\3FGL_prob_cat...'TTYPE1  = 'Source_Name_3FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON    '           / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Signif_Curve)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'ln(Variability_Index)' / label for column 7                          TFORM7  = 'D       '           / format for column 7                            TTYPE8  = '500MeV_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'HR12    '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'HR23    '           / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'HR34    '           / label for column 11                            TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR45    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'Category_3FGL'      / label for column 13                            TFORM13 = '5A      '           / format for column 13                           TTYPE14 = 'CLASS_3FGL'         / label for column 14                            TFORM14 = '5A      '           / format for column 14                           TTYPE15 = 'Flags_3FGL'         / label for column 15                            TFORM15 = 'I       '           / format for column 15                           TTYPE16 = 'Missing_Values_Flag' / label for column 16                           TFORM16 = 'I       '           / format for column 16                           TTYPE17 = 'AGN_BDT_S'          / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'AGN_BDT_STD_S'      / label for column 18                            TFORM18 = 'D       '           / format for column 18                           TTYPE19 = 'PSR_BDT_S'          / label for column 19                            TFORM19 = 'D       '           / format for column 19                           TTYPE20 = 'PSR_BDT_STD_S'      / label for column 20                            TFORM20 = 'D       '           / format for column 20                           TTYPE21 = 'OTHER_BDT_S'        / label for column 21                            TFORM21 = 'D       '           / format for column 21                           TTYPE22 = 'OTHER_BDT_STD_S'    / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_NN_S'           / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'AGN_NN_STD_S'       / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_NN_S'           / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'PSR_NN_STD_S'       / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'OTHER_NN_S'         / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'OTHER_NN_STD_S'     / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'AGN_RF_S'           / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_RF_STD_S'       / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'PSR_RF_S'           / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_RF_STD_S'       / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'OTHER_RF_S'         / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'OTHER_RF_STD_S'     / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_LR_S'           / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'AGN_LR_STD_S'       / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_LR_S'           / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'PSR_LR_STD_S'       / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'OTHER_LR_S'         / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'OTHER_LR_STD_S'     / label for column 40                            TFORM40 = 'D       '           / format for column 40                           DATE-HDU= '2022-01-29T22:25:49' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             3FGL J0001.0+6314@]RÂÀð ?íŸWÿÎàVÀ9ZzŸÙOÀ:ÿ!Z³¿õÆkvñxÿ@Å "	¸@ܾßú&!¿ç0WìPӿ쳊Ügu¿ÜƒûÂكê¿îæý/k'–OTHERspp?è ¢+7ï?ÈU6Ì?–'ë;$%?˜Ã{Ôz?ʺ¼K»¾?È MªÃL?Í#¨IÑ?Ô£\¼qm? §p|ry?«ñÓ±'Ù¹?笞ùµód?Ô5D›'
?ãÝ"Çÿg?·["p‡÷:?¾ÒAéÀ\u?¤ªüŸàP…?Б+sÿê?µHƉó¼z?ì+‹þ´P?±M^a12-?RÛ))ŠH?Z>GôO†?¾\û·[?±I¼ü¯Bç3FGL J0001.2-0748@VAk¿×ÀPÔÀ€"ÐÀ9"ñóÍÃÀ;¯Þ>Xˆ?ä‹|¸&;@Avû	 @1݀#Pè¿ÔÇZö#eé¿ã+ùÖζå¿Û5šÜdÅR¿í›Q÷æÎAGNbll?ê-ªT!ë?Àu³ƒ³FY?¼ÉŸÆY?¸Z'^Pã?±É
˜—›º?¯Ú

W|?ëè[?»œ¹îåº?¦'ú!hƒ»?©øúÙð¸?µBùü{T?³LAMøæp?æû6¨àw?±º†ùúÏØ?É*CAÇÀ?®GÇmb¡f?µÑÄ5n	ÿ?¡uPyK á?èµðŒ~ó?°´†Šèf…?¦h2(¤?œb¹²ä#æ?DŽ#Á€¾?¯ƒÎo³3FGL J0001.4+2120@Zê–_RuïÀD	@¢CÀ9‹!P²ŸûÀ;ÎÑPÀô?÷ÁF#zÙe@{J¨š¾@d´¢´uh¿ã©OºÛç%¿êJJAuHà¿ïÿ:ÕÇ?º{	¥_rAGNfsrq?ïôS#–t?cyV*À²Á?CDꑛ«Á?Uû}ÖzÙ?KnÔà
ƒl?U¹}1@?ï«]_
m?ŒúYÉX?Sõ†èÐ'Í?o.'vYŠF?'©ïK#_D?†þÜ|x-?í
íšD›á?¦0Ü
+e?¦ËêtåÞ#?œð<1~"5?¨…;æÐc¿?Nú¨í?ï‡rÌMÁ2?"{¡NxV?cv¶c¾0ã?zžåñn#k?‰EŸS 'D?"5Û\s3FGL J0002.2-4152@tá !¸ÀR	"`¸À:†¾š§·À<˜¡L'¿ùº­ Œ§ï@ \2°@¶ÆCò¿éÖ%8ý*@¿çž>éí‡?±Dņ YÖ¿â"yq…ÿ3AGNbcu?ïüöÏÄ'?XDÃø"òÜ?X,ÏN®Æ?W 0ÕÐ2?0sv¬#¼?3kÖä¢Â?ïÒÆ¡'š?y®µÛS"?C7Ô·´3Ê?OˆàYÛvl?t5´Õ:­J?wŽþkÜʒ?ïg&î…?€Eû'9û°?r,ò"QJ¢?bg
:mÔò?"üú¶÷?}¦Ó:ƒô5?ïåfìlÂY?f-¼šÇBí>»ü£ѳÈ>Ò⼜"¤?j•"þÛLz?f+u«Z<3FGL J0003.2-5246@sïž?»×²ÀOiÿ¼ä!À:‡¯»DMÀ;èK	éÎ¿¸otpl@€Ä©Ü¡?þRÅ؈B¿ïýñ$yœ?ﶰÅýr)¿ÙjÓ³'	¿Ý¾_îõcAGNbcu?ïùQ¾Å¸ÿ?Eñí:I/?2l[p?ëËڇ"è?G'·]º¯?DúB^G?ï¡UAÅá÷?–ªZº,=—?d-Xâl?Æ»CnG¼?'ŸY]žþà?‡K6ô3¯?ïBs9àË?€µPú\óØ?|µSž˜4©?l.ž8ÍôÑ?"Cö=ÙU?{x­"ˆ?ï‰tÉՄ?‡ÉV-ŽÃ?n©É¤¿O?p^Ozq?…ø[!o'[?…¬‰)Ûô3FGL J0003.8-1151@U¤ YÀQÅcÿï9À:¬"V;uøÀ;ù è­Óã?âŸ8ÅCk@
¢'<@0+ÿ>l?éyÑyý‰¿ØóK^¿åD:Ï<q¿Ü¼ûßðýAGNbcu?ïâ­ñ@7?ot¯†ñ:a?`BL( N?h¹ø,?[^ÍhT.?^Ά}gÐx?ïÇž§é?Š¨㾉?]m%Ù"!^?aòÇUWê{?ˆ`s¿±Á?ˆ×•~çc?îhò¦,¿?"8䀗£q?—F&¾Cç?‹§ÂðŽ_V?››"|+àÞ?…Ùç»d•u?íÐÉDá‰ø?¥XÛx¯Ò]?ƒc¡iAö?…¡Äy©GÖ?®ƒo
?£þ]ûêÒ-3FGL J0004.7-4740@t=Ÿ¶MÀPá1ÔÌvÀ9iÎ,H]gÀ;؂—õT«?ãqP7®u§@è<Vžó@:f¿§ C¿áMwé+ä¿æXÜZ½³¿äXzLnºë¿ïÿð¸å9UAGNfsrq?ïé4v²?hùêè]Œ´?QRùÌÖ,¥?V²èIõ?\DFps?c÷ùo«µc?ï/Ái¡<?™…4z³è?ré9†Å3Ï? Jpô?•M'Q‹'?"ù(¿õÔ?îA1Ã—?—Â+ið;?žY"÷‹-?'xÜxiB?™€LS¥"?‹»ÓW9?î9–M—´}?¢Ècbÿ?ƒ²'ES?‹×EE?§zÁà¦ã? £K'\ßÂ3FGL J0006.4+3825@\U=žÇÀ7‹@;À9Jn¿Ñ;ÇÀ;™2"Ѽ?êXyç¼V@&í @ïဎæ¿çGkÚ¢+¿æÝH
1ÿìNC–œ}é¿äz"&V½AGNfsrq?ïôø1"\?Vތ‡¯h?LB_ÎNê‹?PɏC÷??¹³ÃDÖ?HÈ}œ %?ïʉ•'?¢žêVù?}"‹´(çÌ?…²%7_€?–¾òã!'?Å]!ª{Z?îæ¡ýpé
?Ç³Á?‰à¤Ð»Î·?§'™ D÷?–;mé"÷d?†ÐçR?í-cÂ2K?§Ðä‰P¬a?—ôÑ Î?"úìº½P?°—Ýú
»d?¥}µþ>Æ3FGL J0007.0+7302@]ê_á'p@$ëÎ ‰ãCÀ5"á÷|þÀ:H!ß&¡@ö%/Íù@¨Œá¥Kÿ?øè!¼é)û¿É_:@KRA¿ÙyB+s¡7¿à掝¿êwë1olRPSRPSR?_c"·ò²t?nȥæ?íh †9Û³?¼NU¨åÅ?´AmQW¡?¼ã
«á?JÙ	ÁEE?5P¤ë*
?îð¦k)XÕ?¬ Ÿ€ÃÙ^? Š5&f"?«!E©7§â?³ ¯£N)Ø?¥*ßäI‹?ä<š³vÞ?½Â]ÚfrM?Ҟž°@[Î?º&{cc_?'*Ý»«3¦?0U…ˆo?ïNíGMå?'yÀ•ŸÛß?•ôT^ìý?'`ÌPtÎ3FGL J0008.0+4713@\ÕH˒:À.WÊÆbÀ8‹e²€gÀ;<µgUy¯?íñvi,®@Ó=…Ï@+?ëÓM¿ÀvþF
ø³¿àœ €Ò[¿Ú̀èYˆ¿äC9qzAGNbll?èýPìH¸?Á
-Ä?G?³¦nèhœü?±ÌLöD	?Â7ˆ,Ž£?»€§4È?×S
D`$;?Ëþ¥óT?ۜÜ:–ù?Ê.ŒÃiã?Ê 3{•?À²'‹–»ª?é†ûG»sŽ?¬_#ޘ?²û'ûc^Ö?Ÿ»o3Ã?ÀfQc`'_?¥Æ&…Uç?Ô¨ÿò\Ç?¸Ê¹0?Îé"Æ»?½"…
÷"¬?ÜH'—Û?»lRüÎ3FGL J0008.6-2340@I#ڿԖÆÀSð*ùš‹À:c)ÒaaDÀ;¯S;ç6Û¿Äû¢£-—@ÜAƆb?ù•<@5? °ò?'Õ?ïüz¨£Þӿ窜>öœ?Ú£¤6¢ö²AGNbll?ï¿^§€fó? ¬mš.½¿?QÏ¢¬E?TÒdÍÅ¥?{Üû¡u.? ŸÛÌJmŠ?ï­[ˆŸä?†Ni2‡Jæ?F#¡÷Ó?`…[e®‹?{é-ÇqY?…ox9–ÆŽ?íñp%—I
?™?Ý{cß?žú¦VU?'çŸÜâ'?¡k÷S`dú?ŽçÌñ¦?ïÎwã°­?}ò4èÖøZ?B¦ù^3'?Z½VžÃ£¿?vo/Fd"y?}>9Ç t3FGL J0009.1+0630@ZMa²¢ÀKlR@>´qÀ9Íêï̓À;µþÓ°Ý¿ïæJ˪@w"²î'@oV@S'3¿àmíóQá¿ã-˜û¿áW¹aÏÿàŒ*h¼àyAGNbll?ïÕQÜ‹?u–†ÀÞ?7@¾¢9×Æ?6 Qþ®Þl?sã+§–"?tӕ¾Ó‰?ïÅ!ü*?zQÿ7ÎU?J|Rµš€(?Tbµ?óÄ?zò«7¥Å?wyOÃÒ0*?îï=N ?ŒVª}íå?…N5²FÊ>?xã H$¯x?—q;bÙY7?…쵐ّ?ïpŽ‹¾Ëk?'ZŽ
52? dòÇry?ñÁôû$?'ÖŽ#3ËS?'D°žp\33FGL J0009.3+5030@]s`Iì³À'›I ÛAÛÀ8ҍÖí¸À:ú€ÌC:?èNêj±="@e鋁 ?þÛ°àˆŽ¿á"¢x1¿Þ&úÓùÅ\¿Ù͹"¤³¿âQ®Ñí§AGNbll?ïîªV®¿Þ?jË%é?!ÜLUôG?3ƒªÅK¹¨?`7ä‹àßZ?i†©?%?ï,Ú2€è+?¡ZêÂVB?wß/ØÞõ²?ƒ?O<Ÿ?"lí¹«=	?œ»çÜ·Õù?îv/&0È? š˜1¿?‹ˆŽm²Ñ?"y½˜{?§öyrV†Ô?›±|ÅcÜ?ëžÌóõoQ?¨>£ªÀÆ?|Âm!3<—?y!F;$
E?Àž¸Ç ¨×?§ÑîÀä¥3FGL J0009.6-3211?ôÒÆ>¾ÀS愠
Q!À:iÁµA•ÍÀ<YQªí?›¹ÉŽ©H@™ÎØÿ@zSŸd^Ͽ〠ƒ¿ãô](5dw¿æ¶"Ò
¿äbzª¨hAGNbcu?îP¦
Ϊ?±|D¢Dü?r'›€-þ ?rwiJPG?¬
¢/U—?±H€JëÔ?ï1gKé§Y?ŸJŠ.?gKÀN"?uEXì-?–養ÁS?,"{–þÃ?íWÖÇ'Š?Ÿ•pGÇR?™UEJH?…å~­Ù•?­ØPè}Æ?™ã\â)۞?î@Ó,Žsâ?™ÏÈÄp´w?rrÎèÓd?nŒQTµ»?©¤sYþUQ?™;«ÝÉÛº3FGL J0012.4+7040@]ëþ?5Ÿõ@ Ì <ÁÀ9Ê ™ÙZÀ;KÀæå|Ç¿ù¦®ÕëÚ@‹`Þj.@Þ¸@xÁ¿ã
Q2L®¿ëÓP¹?
¿â1Àª³%¿ÜGÐç—1AGNbcu?ïBq]³É? ¤ØNb:?@þ9§BÊ?>Ò#;ə?—)â'/p"? Šæ¼"Z?î>-,
»?µ'û?Ï/Ÿ?p"—ó>ëÈ?x·~¡éƒ?­éª.×vâ?´ÌƒÎäßð?í*%-þÔ8?¤ÐïKßíJ?‹ÔûAb×?~"Ák®(?²½[ð¡1Þ?¢¯,_ñ?ïh)‰iLE?‡Ò5ÛÁ‰X>ý"7À'_H?9ªK|²?'óiÄæVæ?‡ÐG"š3FGL J0013.2-3954@tÅ.@…+NÀR½"@(äüÀ9¯ó¢#«×À;ÛÞ|!¹Ž¿þ)
Ðx(@¿(Ÿ[z@±»€Hj¿â4¨©,	¿ä+P)§Þ¿â¹).<¿Ös³Èç1tAGNbll?ïÅ¢‹# o?€Ý{Š^?9q~¹|?7©%ÿi}Õ?{—¢'•ø?€IEÊ.Õ?ïÍwF.Z?||¿e@R?Bh±Ý¥Ë?La¯B¿¾?v÷FÆ;ž_?{Ljçsß?î"(í¦?"¡~©©?|?ˆhÆüxö8?vEßñ‹IP? ¤k²`ñ?Ä~JÆS?ïÀ‹òÁ?{xÕøt,ù>ìXm»Íã>ÿÉуX5‹?é¸ÑÏÁ'?{qáñ¼r.3FGL J0013.9-1853@R¨øäÀS…€,á
À:¢ÐqœûNÀ;þ¦Ë±CÚ?ß!0wþ$š@Äû—»s?þö`¾ø?ïøÀá\%ñ?Õæ/–½é|¿ÚëlÌVo¿êǦ—}"AGNbll?îD"uQUè?¶¹ÅÀ)k:?¢HaóÃÍÝ?²|‰è¸Ÿ?'Þ­nM§t?©éOãAÇu?ç¾%‹†z	?ËlÛQà»?½6ÌOθª?À['G,?Âl©þ»‹?Â_)?_n?êVnñJâÜ?®z¶Ó&?¼ñ‹p–¢?§è%9Ãñ?°ZýRƒ?coåÕb?çwŠºbn?Ãhýt?Ç¢d³Tªð?ÁÛÞ՘žx?µCƒ–¶?­‹¼¡¦pö3FGL J0014.0-5025@s×7À*ýÛÀPh"  0øÀ:™û3èdÙÀ<0{ÈÎ;?×Ɵw»3®@±Ëžðñ?þÈ3€5'¿ç§vóÁ.¿ÑÔ'54P{¿ä/çP~$¿ÜºhÆïƒAGNbll?ïÕ>²°š?ŸvÁÁ6ñe?dƒïÞö۟?ŸgmÒJh?f=€nX‰+?kI§a"nw?ï‹òi‹€¤?'‰?
:ã?YeÔíÀ?_×÷"Qî?‰ÖªÿgÔì?Õv¤0?îÙNo¶Ñ¢?‹"[Ò6ÍÝ?ŠLŸ˜Ï-ñ?y<'ñÀ?—¯â<¾4â?"e«b"kh?îçQÁá?'ítµ#?mcv€£ü?o(¥Þ¼`?ŸiY¯^?'2µf–•œ3FGL J0014.6+6119@]¡ñ'l¿óÑ=ŸÈ²·À9"=ëóفÀ;QÙ($â8?ìqÌ[ã¬@k¾vçÂ?þ3#Þ¬s;?î'NË®Ùa¿µ™^'Ÿ"¿ÑÃñ)è ¿ÝWGph.#AGNbcu?ï5[|5?˜"+'~,1?'E1?x¾Ò>?šMÉø"?•£.¿FW?¥£‰—©?µSRšV¥?¬luÅ /?°0]"lž?ìß
-%d?¾.oøí?ìo£¼·+?£d÷É¥?¡,̺n?Ž¤S
_êŠ?³ì
™ép? ƒ'*ß0C?ë'¥PÊL?±Í½2Ñ÷?œï*Ú.Z?˜/_·8?¿Ð î?°x$n	s/3FGL J0014.7+5802@]"Ñ_ÄÖÀîQ`Dä6À:.[)òBÀ;'Y5%{»¿ÙN´þúÇ\@
i•ûg¿?þšåŸ¶´?퐗Ã^B?ꎽ¢ãD]¿á>Ö¿áA"HŸkAGNbll?V+ýÜ?®Ïf‰f??kˆxM(—\?o`tº±A?¥k³m˜¶?®AöŽÙ¼"?èoX ?Îÿ~&uf?§ÊÕGuq8?¸VåQÀ…u?ÇÙðÂ#R?Ê8[¹¸I?텛ÉäY?›)ÀãçmÑ?˜¸;ÑQ?…߹ם˜?«J%y*Æ$?–-"z@?ìΙÊ얲?´üÿüèlU?¯'GÄÊ?³aIËí?£"Œl'Í?¢©ª[Éô¶3FGL J0015.7+5552@]z,¾¤ëÝÀ˜>àŸ°À:])¦ÂwÀ;§UCÿ3?¥¼RX‹‰@

a'Ñ×@êÀ/¿ã•ÖÞ¾¿æ®ëFÏ6"¿âªƒ&:§F¿âÓ´`ÖjÁAGNbcu?ë;þ÷?¿@-WbÎ?_§çezü?a­‹°²ñ?Á‹Ááé*?¾ÓÌ">a3?éĽMšé¦?ÄH›ÅBÂ?œ(·Äó? î	Oʟ?Ågóé;×ê?Á'É)¨?í–e8˜ýÂ?›7\ÿ£l"?"Ñ5¥ø…?m/'SÄ?¬±ê'ž?–ìÖ·k=ú?ì^= Dñ? ùÓرg?~"àÜ©
?wÒÁˆs/ä?»-©ÁØ
è? ÀWµò3FGL J0016.3-0013@ZáuÑ=ÀNç…`&±EÀ9;ŸDÔEgÀ;¶QºÝ·?ó¢xËmÒ@±vÚý½@ñ]À¥w¿ã¼²Læ/¿éq`œfÂF¿í¨Âñ¤¿ÖÆQ÷!<ÄAGNfsrq?ïíøîÖ*Ñ?q׸Wf?JãNZ+Æ?U3ShÃ¥?W
0¬}FÕ?o€`CK?ïÂ(ˆ²A(?¼k8Ó?K`nŽ¾{?Xˆ¨¾Û?¯?{­Õœ?€,-9ºE?î^÷îyrM?˜ym%R}?'āv'Œ¸?ˆÊx÷ÍG ?¡.@]UÙ?"Œzø?ï>n ü?™ݗ$]v?`Èòn®?jfÚôrÇ?–#-'®?˜¡­²Dí3FGL J0017.2-0643@XêÉ`0Â@ÀQSÙÔóÀ:*V]çÀ;Ï% £y¿«NÐÅMŽ@øœJNì@íø@˜÷]? R
Œçã¿ÅrdgnàD¿æhuµ8Ü¿è¯4Ã×ßAGNbcu?íl@
JF&?À;'Ýã·²?‰Žò±Ž}ð?›	ÉN"Á?±l!W{ÿ?¿
öúgž˜?îL@Æ£?¦‡†
mVÌ?‡Kq…¨€f?ÜÇ?›ø÷?¡Xb‰u©?¡/Š
ýÞõ?ì쿱³ú?¡OG;Äû?§àù"ÛE?˜ÇSs³¿¡?©]ªp	µ?'i-äùrê?êÝÉé(b²?°{E­¢ƒ|?¨Zõ}m«?¡Þò•_?¼ä­;þ3£?ª'ÔBE¯3FGL J0017.6-0512@YPŠŸb0ÀP©&¿òÉ·À9)´xB0ýÀ;cî4üa?ãÂÇàÔÁŽ@Àù™´qŒ@áÀ#ñø¿äÜEZ…»¿æéú`"üb¿êvºÏý·¿àÏÀÙ5AGNFSRQ?ïú>츆n?AŒ]p/™?*©Ì!Vˆ?)©¦-*—?@Yڐ§?>=	vz?-?ïÔë讵_?wà÷Ôt§?CŽ +™K3?O®û-°Å|?s7£2'+?u£½Ëá?îÿlñaÛM?ˆÁdFÍî?ƒ°¨ætO?xGÿwÿö8?–:
`¾ÜG?'·Õ3[Q?ïÆBV¸?y¯
gúïQ?þøûŸÖÌ?%ô½jŒK?|†Ù¥?yžŸK—XO3FGL J0018.4+2947@\›¨d©ÎÀ@Dߥ¥À:´Ÿê$ÌÀ;ú"#—µÀqÌMËåÇ@r÷na?ýÕ
ÁÉR?ìQ+êr,Ì¿êàƒKà^¿ÅAí§"¼¿Æ(·±TÒAGNbll?ïü¬'d?@v0I¼W>ö2 èHW>óRޕ&f$?=÷{"й"??¶øâÉÁ?ïÏcÂç²
?uâ5¾G ?FÍUNðqÃ?Nv·~¬úv?utsâHìr?súæ8°_­?ï=Ž³ƒº?†pIæ/]ó?x3wå‰Á$?qtv́â%?'QP0-‹?ƒ–É%±=?ïóøÌê?[f+w»wÀ>€7è«\r>'ªø;3à?XQè¦çí?[eæ\ÞV33FGL J0018.9-8152@sH _ñØÀA"á@!X?À9¦8‰´IHÀ;©‹K"=B¿ò½¡ÜF@ÍnkB™@š€ ¤OÖ¿å¤püÜ#¿å¡g÷¾œ¿à–hjU;ú¿Ñw-HrAGNbll?ïör"sòÀ?WŒMGUN†?þ¿@N®?"Vø!M?R[Á?VúùÅÕÍñ?、lXB?yYð–ªÁ?Kq;f¼@?V8G41ȳ?{3gq?vpô†3Ä?ïX•WÇ;!?ƒÓo¼îÆ?rD-l""G?_jL§ßâÆ?\I¬öÑ?'-97Ô?ïßúm3u?gNZҔAs>Ûi·xj/Ú>è-©k}?px([ˆ*}?gF_SÈ33FGL J0019.1-5645@s{´?¢­?ÀMéE¿ý±qÀ:OÁä;~[À<mùÞý¿ä ìî¥{@;N	Î5@  €´ã¿ì;—"°BA¿Þ݊t¸Ž§¿ã'L]"H,¿ÑçeÈdeäAGNbcu?ïøÜó€ý?Q4;DÎ`?58³pÛý?>|»'§?AïØCžSÜ?IŠŠä…Rª?ïÏO}åÈ?y/
^ýI?DÞ ¶î¸o?P*8è´fõ?u¼|ö>"ð?vüQ¹2)]?ï>.¨ˆÙ?"=ß_ì?ƒú"~_ê?z»÷‹¬v?W[»|j?yêäÛ«/«?ïÓE|(s1?p~ô*ÛÌ;?û‹|–?¹*ø™>7?v#JÕ¦fQ?pfD]ED93FGL J0019.4+2021@\5ý~E€=ÀDð[ÿÛÀ:dZUÖÀ;ã]9–û¿áÕå
C@ñxô@ý1 6ç?ÚHtŸ|¿ë¢CgÄñr¿ÚESÔ	úL¿àû7Ê$Y"AGNbll?ïû-ë×?Bæ<0ªˆ?lèÅô?'}…Þ?@š¶ª¨?A;íM€Ë?=à$?{ó‰bm†
?Kù½¿Î]À?S€ú~žÿ?~1Ø5¾-Û?yѪŀˆ°?îçS™õL?òjܐ¶*?°z´—6³?tÞЈ?š=O"•»?‰»šcƒÁ?ïtýÂΞÙ?‡>÷ùG'ª?I֟0±?ho&Né?'Eýόô?‡5éJô'Ö3FGL J0021.6-6835@s01€
|[ÀH&a_–hÀ:J¾ò¶°À;ÿBûÅ¿â~Ž,öOŸ@–CPŒµ[@8B«v'¿äé©Cõg¿èÏÎ@F¿çú˜ž-8Y¿ïÿPÓP¹AGNbcu?ïÒTÐû%?©µiž¯Á™?eG\/³? ãQEn³ê?hc¢‰Õ&ü?'ÍM¦ |Ö?ï+íì§ä?™TøUý.6?p§ÓhRÁ?y¡"j‹há?–u­hfnþ?•Ì&ÇÝX?îFëÇA?"ú%g],¡?™Á:ù4Ý?…ìí¥Ls?}âéã?‰˜2ÝÐ?î™Ê¯û}?š—ùí&®?wՓ˜¸Ï?|SjÜÕ½?£h¢šéDÌ?˜ujª÷Œ3FGL J0021.6-2553@Dçڟô&®ÀTÎ]?á—_À9¼º"eÀ;Ζ67Ê¿ûõõuã\@$|>M@ËVß_Ìn¿å<RÐÝS¿Þ®îñËðë¿ÜR¤J«'"¿ã>"¤âD{AGNbll?ïê!ù
‡¤?{º2y0? Á4ñòÊ?#~¸C&#?dÑó°Ù=«?{žAÎÿbó?ïWÙÏnŠ´?£ð›,8;?LÅìc¥Õ=?Zö:¨*¾Ú?"–¯zñ?£¡z{L?ïF(UL?•w@ÉH?vˆX ?p@V\íñ?—93n‹?"˜ ~£09?ïȤˆ2Æ?uá%x^Vz>éÀ²ÇÈU
>÷?'cjÊö?{ Û¤¸¥?uÝÊîÊu3FGL J0022.1-1855@Tû_ò®ßÀSØÊërªÀ98?±Æ·	À;NQ"GJA?ìˆÓY'Ž@ÞÊÏÇ~?üÈÇ>Ã_;?î¯ÎE.¨¿Ø.¬Ï¿ÐìBÅÿ坚ݼ^@AGNbll?ïíö4‡ã?bá'1ԍí?DÌ7µ]?CùÊìˆf?[r	{¶T?``:ý3?îÎý DG¸?­v¬Æµ·?pœ<œÐ»?v;{ÔøF? ü¦kÇêq?«ý¸•6
ˆ?î^1bpÛ?'>ƒ/Ë=í?·÷ò61?ãÀ£z¾?œx>I8ɑ?Œðí=¯n?éEJõ"à_?¶÷¹='Rå?†÷sU]ó]?†ã©Apê?É{\ô–ŸL?¶µ9
‰
F3FGL J0022.1-5141@s™ìºËCÀP4߀-·ÉÀ9'컝oÀ;®,nóÓ¢?áDÂé–~@Vál)?ÿ̅>õ!?Ô.¢)àú¿ÙݪƐ¿æR¢¢Ša¡¿Ð0žú'¾ðAGNbll?ïÙ§ZKæ?q—"•ë1Ÿ?b‡õ•¥Ñ?e8ñ³øT?cаbJ7?e'؉?ﻜ‰Ó}e?{ёyí?M'\"?S	"dœ¹^?~—ÒuÊ"?€OôԊR?î>gøòù0?–QÉøÈf?œ¢c‰º?ˆ>ÃC?›Î ?Š"Û^ë±Ó?îè(eë?¥6ýUF?sðŠ¿•ŒA?zª•?«£l'ïÅ?¤i>£¦±Ä3FGL J0022.5+0608@['¾‹ÁjÀL V·À8s¹NjÇÀ;:ÑY#‡Å?ì½Ã²œÊÑ@9aÜ>ò@–_¡PG¿Øÿçƒ~Ç~¿âœ§jŠò¿àjT7˜PL¿ãi,¶0BAGNbll?ïð»¯2#?p…Þã%‡?*ä¹ù+ä`?A%
§4
o?[-ebv<¼?npÅ2 ×Ö?ï[r˜PÆ!?–øÉ*e‹S?k‰PÝÕ<?€n•O&ÓÚ?' 'õˁY?'"¦7m·?îWÕ°°?špÉF‰?'	Tw¿?†ao"ÁÜ?¥…Øiü|?•Þ‡à¾4X?ëKoVB?¬²Cjï~?
OköšÈ?|™³2)?±ýKçŽB?¬t»ù²ä3FGL J0023.4+0923@[Ý? §?ÀJmÎÿ¬óéÀ9¥:¿ïn¸À;×Ájî‹?ûðT5:Ÿ@ƒ`–mÀ"?øbÀú†™b?µ±¬lÒ]¨¿âç·¬ §7¿ìÒÈ'²²«¿ç…¨á$PSRPSR?Õ}£ÕuÕ?ËAV­&t%?Çë%ß	?Çaæ…kÊû?ލb—š¦?Ðû¢Îµuq?⍈†ãSÌ?ÐË'(ð'?˧©.RÑÙ?Èo%'8ž?Ê"4¶Þ÷?Âø£íÏå•?Ú8͔6}?¶®8"'è?×ú}7êí?¸…R¯ª?˙jÏ#/ë?°ª"KÀ–Š?Ô-ër?ÀWTþïã?àÚÊ|MV?Æ?¦ÿ£æè?Ç>f 7æŸ?¾ÜJ˜|¹3FGL J0023.5+4454@]oâއ	tÀ1¯X?\6bÀ9 Q¯<ÜÀ;¼fÉbµ¿õ°¸´çÓ¹@ú@'7|n@ŒF JÎ/¿çôª}±J¿å´³5ˆ¿è¿`ÉLc¿å¿½Ù{4AGNfsrq?ïñ.u̒5?YNÏ!:è)?Côúû¢?Cæ>­Mãæ?S©i]ÃW?R¦ý´½µ;?ï´\6"?Åœ
}?YPÍ­;vý?`{¤Y3?£žyfÚ¯?Aù'"l?ï=…¹@"2?lÖý#hæ?{Ä`Xt4…?jNÚ½T§Î?'^0ÁÐl¯?|èÌ瀼?ï<â ¡?'‹ù,C¶?5¡_–Mîó?ErÓ³Od|?ˆ¼[K¨?'">5êŐ3FGL J0023.9-7203@s©_ªŠƒÀFs¡€èTÀ8^½ÇvK·À;f-ù7Žã@¶@)æ®J@ø	24?ö"»J}¿µtDJ‡¸œ¿ÛÍ:°ÕöA¿æš*ž9;‹¿î#J]'OTHERglc?:Ë}Š¸??‡™Ce ?ï¸ôl°?‹"¸U»?€ìˆç«år?ŠºYæKš?`H³19Bœ?s>éûŠ¥?î´Qoþ¨ú?¦OIô0f?£¶]ÍÜR?¥Š?(ÉúU?‹q{Ž{¾?~øDLcÕÁ?í÷·õ´Â´?—–i©ªÇ?©¨<EÐ5Í?"£êÅBÔ?gõðª
~w?c¹'èyú?ï
ŒÏî†?"Ágh‰N‹?šPÀ߅?"™"£g'è3FGL J0024.4+0350@[M–ÃüÀM,Úÿ•võÀ:Þ
ò}À;¾Êe€?ðAUÈ3‹@DpýC77@9ÎÀ—à1¿àëÝ3L]§¿æ¼,ÆÝt¿ç¼æç;t1¿åÀ|µ2AGNfsrq?ïÆäÿ·ý?˜±Œ.RV?]äՑK»S?d,¦ºÆ¿…?uwXÑï?˜e\·27?˜&Óö?™"l‹¥?bÃ(̾ù?fÔ/fðü?Š¨ÏðWÓ"?ŠŒª¡þí0?î#a:gw?–êê+ÖÞã?–)hŒ‰Cá?‰p{e?¢µ9ææ ?'{9Þ^ÿ"?í}n´ôEŒ?¢tÃÄë?ˆU7
è¿?…ŸgØž†?±	ãwV"?¡'øpù:3FGL J0025.7+6404@^@¿ã°?õgq¡-ÒÀ9Ë/þËLšÀ;5í£ùo¿À¤®'À•@Œ-ëÉ@±§¶Cž?ëÿ&ò³¿çú
½'×á¿æ;×F£R¿Åoúä¸%÷OTHERsnr?ìʵBî‹?ºÕ°½y?Š%Ÿg;?"iÀ) æ?¶fñ8¤J?¹ÂÛûdõÀ?ÁYGT¥? ?ÎÚcüÀ? '°ÖA[e?«Š}ï™o­?ꡃrš€?Ϻ–bˆîË?ëIÙÖx˜Ó?§"iÍ@ÛS?¦dâ†hŽ?•žÐWÕH?º~À	9…?¢öCæň?ê;Âó§c?·<˜ž+¹?w–`|. Ÿ?ÆûŸ_
I?ÆTA-€þµ?·
#qˆ.3FGL J0026.7-4603@s½¿ "`ÀQœˆô'À:'–Æ€'qÀ<é¾u5¿ð¹1ø¶Õ@)v'hO @šK`%¯'¿â·4¶&Sb¿é'JO¯j¼¿Þú†¡øÁP¿è.4v)R	AGNbll?ïåù"ÀÐ?y	i(
ó5?.Æ[Áƒû?:6A¤ûð¯?hwŽoç?x¦šA2®1?ïÄ9öOó
?{xuÞââ?E"P29^º?O´­	¢¬?{0šÑ¿Mû?y6–
mjù?î–_Š¥?'ÑFÁŸ'a?…9Ù%ƒ¬t?wŸØÀÍ"?¡K'N]?~¼€
œÒ?ï¥b¹5VÞ?}#" ´¿k?ÍÇ5k#ÿ?ïá†<ýÂ?†¶$?r5?}nØek3FGL J0028.6+7507@^[òà\̊@( Q¿æ4}À9µ´v"±ÓÀ;™Ž"¬Ï¿ìº+­Wçs@
~kjÝ@»M DC&¿æG9H‡>‰¿ãÄ`óhu"¿Ü`†ÜX¿îÈ·ôoöTAGNbcu?à‹R~"?ËÇßåI¥?Ï¢tQJ?ÃüœG8?η"Z•\?Æ\‹'lïU?鄾–¤Â?É£äˆZD?«I¨ÙÒ?±Û«ÊFê?Ã&s;6ƒg?Ŏ§A$þ?èöðÑ?°lŸDm?¾hòcá?¦•€$0?»z1Î|}—?£íß)SW?ìU_ÏE,?¬•—ˆëŒ?ŽŽÀþ÷?"_—3ó?¹ƒ)e÷¾|?©é \dsý3FGL J0028.8+1951@\ë°À&ÌÀEYÝà‡kÀ9üaCöÈÀ;Ë«Ä>ˆÒ?åÉoïxð@šÀ`-@x+ßVè¿æ‹ƒˆ±¿à›º%'p¿î°-ʓŒ?¢MLu4ƗAGNbcu?ì,±û>¤ü?Áüށ²½?­þã3"Îä?¶võÝzù?¯5ýòáe?¶A€c—•?ï -/?½Ï?ª=§¶¦_:?w?³²ù?"³tÉ*?–3وYr?¢RB®œ¨!?ìœNBn?£Ð½˜%9?¤ÛrÚ¶'Í?":í)õæ?°±Ô:ت?€×·äâ¡?í®Z|ê#?¬›"è?"ñSv÷$?¡GjÇMQ?«_‡£¢?¦%*Kö"3FGL J0029.1-7045@sKÀ]RÁÀG!?©c;À9Žslf×À;ÂDw(UŠ¿ß:]¦Ã@>-_‰¨`@F±_ˆü"¿èm:$¶e$¿áBf=1ö¿à!Ô³mx¿çbN°«ó¨AGNbll?ïßz`ÿ?i½—89Rc?F5²ìõ?GÛ9‰¸è?k^?QãÄÄ?gRM=èk@?ï£bê?ËcO&0g?UJéÚúÞ?Yø/ËL;j?"~7>_?€|/nlœ…?ï ‡gª±x?†=Îr'n¸?pùð~ç?qáWΈº?"6–±'‰?Âõ†r3…?ï\' W|ª?†˜Òqu,?A¹ÿ¦}€?Aˆ'¤˜V‡?"á®%6Ú?†@ƸLÁ3FGL J0030.2-1646@X!T€uÀS¢î «†À:ÆÌ؋GÀ;Ôač?Òd
VæÓ@§rëZ§?úZê:GÏ¿ïœ Rc'º?ïÿ™¤ðÿv¿×mÓôv¿Úbêc",¦AGNbcu?ïýJ$¤Q‰??XŠ€€¡?caHÛ?	N‹/X4O?3N®qJ¶µ?>š™Ým­±?ï‡ø;ÏÅG?—(¾,%ŠZ?[&JV ?|•¬½«ÃS?Š'ºë—?"²'Ò<BŽ?ï8æÝщP?»œÞ¨?|8XŽQýÿ?|æ'3aÓ?'Õ":Vr?‹oÆi¯?ï[Ž¬{¹µ?"®'FÚ?að%Ôý–?e½o!äû)?'P'+Î)o?'¦Ãoæt3FGL J0030.3-4223@sÔÖàL'ÀRˆð€0<À8¥§
›duÀ;¼^¸; ?ÚJ"Õߒo@‰«Ó
@¤ë€—.¿åÚÎÙ¨Ž¿æÒhõk¿é•";
ºf¿çí)]5TAGNfsrq?ï÷·œˆY¦?^ʄç)äÅ?:ßüä?@§/"B§?DÿÚ)l"?[[ˆðtUæ?ïŠÛL¹à?–ª6(
2±?T˜JdÊÍÎ?b­›wì¶?Šé¿à8.#?•ß¢˜WÜ?î°|#⅑?'""ÌzTz?ˆ#c$Ç?"…Y<#?ÞúÒ$;{?ŽAb™T	?ï<¸X|¸S?—¿Ì›á w?Zk"ÄŠÜ?bÚjÆ<2,?–Â<¤(
?—=Þ¯ºm3FGL J0030.4+0451@\Ie¶™…ÀL͵_ȽtÀ7††*QbÀ;8k)«@­ï`J˜€@:֑ó?ÿ,-Z+¿Á7#§=àпÞ°NxR¿çîßNã¿î&Çy­¦PSRPSR?f=Ë¥ÎÊ?wö¨ËÄD"?ïÒQKH¢Š?‰t¶Ü·øQ?gpéf£?æœâÛÄ?t}¯$Y–?Š"­@Öãì?íù…B]r=?²Û©á+?­×õù¤Pø?±"#\¿–?›Zڏׂ	?'Ô+€¾_Í?찌/ÃV?¤ f¨Ü"ø?³¤èzŒÂ?¡H3óÒÙA?QvׇN€?Q·b'Í»é?ï~-Óσ?ˆæ~`"xf?ŽEÝÚ+u?ˆŠL²ò3FGL J0030.7-0209@[¶ýŸÓo~ÀP"Ñ¿æ4}À95eWr­À;­7Ÿ©~?òJß³õ:@qa²øe@V_]2¶¿âo58WE¿åÍKaA'V¿æI×é2¿ïÿÒXÛlAGNbcu?ïë•ð1–R?bYRÐí[?Kµ°'K?Jâ¡¿ Eÿ?ZùGTµ¾?^d~:È÷?ïÈ a(Ó?{}Ôÿ
´h?J¹·|6Á"?Ul5ü \j?x˜˜Œd½º?x}ø§~v›?íîÐé]ØI?šV%ñ?¤Aß̍Ox?"WÃÆ=ÉE?™¢#;*X?Š·yNzé?ï½êáŽ9v?€—j«ö¼ƒ?Bõ†7ù®?I®yë—a-?~«ëèF%?€BUjºE3FGL J0031.3+0724@\ŒÿyÈCÀKŽÃ€ðÒÀ: &yÀ;Øöfú
?­òw7aC¦@ù䥆ŒÍ?ý.µÀ@ÍP¿îǨ )z?ëêDE:'ï¿èS´t³¨†?È®?-'_iAGNbcu?ïäl\kf?h<S"Þã?U^ìæ²ôû?_Iþ¦ñÊY?`ä-!'{?_†ÔÁ¯Õ?ï½nL)H»?';KF1B¶?Q%V	Þ­™?_åÊÙµ?|ÿ"hãö×?€6Ì2ö?î˜úìlê?ŒõEMbÕc?]aØ{?]Ë 1?œàã@šaM?…X/.<?ïui)§_?•j*<þ?vÁªšgã?‹QË{Só?‡E/ÀÚëú?†B&=¨3FGL J0032.3-2852@"Œ¼ÀO(ÀU\>ÏuÀ:®1ËT&ÉÀ<âP3ÀÌUàÝ%
@
²gEß]@"! 
Ñû¿Ö{ãaÈ¿æ
8$1Ë¿á¤û|§_¿Ù'ÈÇQLAGNbll?ï*ƒ5n‡?°ŒáiO6?X'÷£žT5?u…:[h?™<IÔ?°l¯™YS-?ïI2W?³ŠžÆÁ?L•çßê?ag©^N?›r*ƒ¦'B?³KqO÷X¹?탉LÒP?¡Šç'¸Í?—ÆJbL{{?‹[J³æÉ¢?«äFL8? $ºJ 4T?ïí¡ŸX0?hÌæOñ:x>š?˜¾T1>Á«õŽI]?b^cç
X?hËê¼Ìº¼3FGL J0033.6-1921@W'¿ö$µÀTNW_ÍÅñÀ84©Tø€À:¯8hýœ?æócm_Á@¬¡fítã?ûo yÒ¿Þ¢þIh÷¿ÔÖhW¿Óëm"ΠڿÖù`ïYÂAGNbll?ïœ*•:r?¢".•?9{ɞÞ7?EJº–ÜÉ?ˆ,æÛdlÏ?¢uóY¸"?ï
¢'lJî?©tâÜtö?]Q*÷¸?d-ô¡Ñ?œ{•ÿÇ1Ú?©²Ž˜Œ¦?ê¢eǔ<?´Áï¿ãÈ?¡|]¹¦bF?•S€-ÖÛ?Ãb^úx}?±­éͤ‰G?äÈs¹
®é?¼á– N8ú?pSÊf¶¢K?yâ֍eÎ/?Ö-ÉdIǦ?½~¾'Ž«3FGL J0034.3-0534@[ß.ßç[ÄÀQº¿ïn¸À8½bð À;›ìVuX?þÍæ°M»@æ`pX,½@%G—ÙW'휿ٿáÕ`•Ó!·¿æA†û‡Jb¿î¨ö4­ºPSRPSR?yÒgbj¯Ô?~AM¾?ïoèhz(q?';Iø‹u?‡²0@‹ñ?ŠÁªÓÔWX?­=í«˜PU?À¯(&Å?és8‹?
?Ç¤(]ˏ?Âz·²ìï·?Á!ºcãξ?¸Hs6©‰?£¾Vl¿o?ê+5HŒ?ªZûŸ¿"m?¶_cI?¡É+Œ¢Ç@?¦‡[÷ÓÈé?›·ó*#XŠ?ëÐ3ö@2ì?®>üωåi?¶:²R"-?¨Mµ®0è3FGL J0035.2+1513@]IP?³t6ÀG»ÒàD²À9OíhMÇÀ;P"Ý?à|[jVWr@¸e{.õa?üç€bæÕ¿ãÓ5»4P¿Ä¯Wíó¯¿ÚCRóà¿ÖEˆ–£+OAGNbll?ï´E7??€Yü·r?QO¦ºý?UZÉhz?€Ë(;g¨j?~՗)3^?ï~üJåU?‰t†ß~]?^>«UÚsò?`îÕéöÇÉ?ŒyÛÿ\_?‡fQcèê?î"+èTž?'{8åÛ¤0?L¤b"Q?€÷â,áÓ?-ޓd»?‰Y÷?íÙXxU—?¡Ì™ÿþÞ£?p"Œdæ­?sèb²;?¶çìz·Þ?¡ˆÇÁ™JÜ3FGL J0035.9+5949@^?ßÖkÀÙß`£-íÀ83J‰'
ÚÀ:õWÁ‡õ,¿ÌçSÐ{qÕ@÷Õ±Lé"?þ]I^î¢à¿Ó}•?uil¿äÔîuOH¤¿Õò™ûiBd¿×á&$AGNbll?ïUKØ$?•¿šê6eï?9‹ØŒª¼á?8KV+.?"ðo"ÈÒV?•Ÿñ4F£í?çh‹J#•Æ?Ñ
ÙRÜ)?ŠÅTOÓÍ?—)@tÎÉZ?Ð&=s×8?Р®´Î}o?êœÀ¥jôý?°!ð¶®î?˜ßTÍQ²?÷݄û°?ÂqЩõÉ?¬ô£"âù?ìäyÚïh?¢m´ñ"þ?E]q«ð¯?J¤I‡'ˆÉ?¸±öVE,ç?¡è"(3FGL J0037.9+1239@]r7`¿]yÀI
Ô¿àU@À9PäEVÀ;ŠG?¿ÕKÐõ%†@Èé¬+—ˆ@6<6[²¿â	ÚIb¿å¶ì"çʙ¿ÝÂÈïiý¿ã&ã
?¸ÁAGNbll?ïá%Ž»G?lù¿}]úí?$·»1ƒ‰?"Gs°Â†?mŽùI9¡?l^[.†ÍP?ï©óX?'´¥~Ú9p?R»6Ïώ+?\0ØUäQo?ƒ+ÑE°
_?€œ!ÃÉ¡Z?ï-Ìû†p?"÷3Côkþ?y¯Np'†?h㙓°o?"Ú«"j­™?'7¾e#C±?î¸Pf—«9?'­°÷MX­??…¨9‹"?Bû×R©B?¤;îF6n?'‹ë×ð.3FGL J0038.0-2501@PÂê /JpÀU•IÿþRÀ9ÀF¯ç¹¸À;á"Év7?ãLL@µ>@«õ–?G@'ã@V²>¿åkñ&!U¿å|CåÝê׿ç¤NyhT¿ìÁ‡§Ý2AGNfsrq?ï«Å	DT? Ý§m‡›"?[&Þ¬»?x"ØáÎ?©ß¨+³Ó?žâ·›Å—?î'ȸŸv?³õ° â?cÞ'ۊ>?n͐_	?¥¥'øOú¨?³­Ë½cÇf?îCa.iJÔ?¡ñrÜG©*?‡ÅW‹yS•?z <dÆÆ?¥Ø—6ŒýÞ?¡°Ü|?þ?îÌäÎìF>?–gýâJ´ä?pçrÖê?h@÷Z®"µ?¡/v"à¾ñ?•–ØÜÿÄ3FGL J0038.0+0012@\ì  ô×®ÀO<¾Ÿã_¶À:[¯ˆïÀ;Õ
»ªeš¿×:]ã¤Ä@'QS"·@@›àEÐo¿Ör:ˆD»$¿æì•^ÃÒ¿Õ"˜Ue§¿åXNRÉP–AGNbll?Ç
Ê^?ŽéËÏ1;?L"'Å'Ð?SÉè ¬ï?‡ÊU!¢?¼p"Í¡×?îâìc†Û'?¨ûUø†+ê?w½Ôm³"ÿ?†áXNd˜/?²þs·¨¥?¥P?<P<E?îUoXO.?'%ÌCö›?'©è"?€'ÎTq?¢'5ìöÍX?‹ŸmÏ )?ìk¹&†1?©üÌ{r?gG:Y·‹?l°9+ûی?»çþÁûª?©
¸—+g3FGL J0039.0-2218@VúQ?ùSÀUp¿ñ7À:ÊËi~KÀ;çåPQQ+?ï¡¿#R%Î@Ë+1¥?ûr"^úŒN?îÚ²ämà¿ág5离¿Ë3^ÿ6Mç¿àÆ<¥ÖF|AGNbcu?ïȐ+<jl?€þg'ºa?QLàôqà3?RŸ»<€Š?wd²$®QÃ?€ZQf'¿?îƒÔœp³Ã?±e¼ÿߏ?wòä•<?"Qι9Š°?¤ÄY¦M1ê?°Êïÿ–?ìÔà¹ßd¾?¤˜"_´N|?¥'-\͖‰?˜çû€¨gÆ?­/Ç<"?šuȁ|™?êù:¹q=?³ðR5Ì¡?Õ[ñ¶þ?šô[´Ì '?¿iÚ§œ?²N³9z—j3FGL J0039.1-0939@\:'@·€4ÀRŠ4fÀ:E$oKvÀ;ß¹Z)AB?í"Ìû=@´¶|ï@ÀsÀ—	q¿ÚR)³W°Á¿êº"vØà"¿í›RÙw¿ïý_"î—«AGNfsrq?ï~>càØ?'[5¦H›ð?xñN(–ô?ÖXw÷'?",?ó~¥?ŒÁ˟_Ñá?ê"Q<_¸Y?ÁøÄ5e_?²î1¼á¼ƒ?³¿;Bˆ×?»ÿD` €¶?¸òvi˜?êÿ`š?ªÙ'.3Ô?¸Äþã¥ØÝ?¢X©û
dE?¶zù!YªP? RÝí í?â\âؖæ?¼ËïV"?Ή=_òÖ?º_>§£Zx?È:"±'?µÈ{ï¾M3FGL J0039.1+4330@^%~0‡‡À3PlÀ»"À:Mq
"À;àÎs•ùÒ?㽝lb@Šz¥7²t?ÿgîÿQ¯J¿éD ±³8¿Á'cÿj¿áÔ?®#ȿݘҔŒê_AGNbcu?ïÞ™™/?häfÏßS?Vþm¬%m¸?Tð'ˆes7?ff0Tå?cΕ›­–Þ?î"¤Ð®Ðë?¯@›¶'N?"*8û+͝?œ4
-ƒ?£À–w}
…?¦n±^CRÙ?î hàT‰>?žÀQå?Žž½WGg?}6§e±fz?œ£…IËQ"?…Õ9çì)Š?íYoÂ((?¡¦ƒ[¯Ó? @M½'j?™òüõ-îÀ?ª(ðzë?™ÍÊ·¬ö3FGL J0040.3+4049@^*§"X¼À6J_Ÿ¢ÈÀ:³t«£‡YÀ;³6nQs?ÔuüÎ-†@HG§‰qX?òºÀۧܿç@ÈôfL¿èXBd‡Æ¿Ùîh§Íþ•?Ôð3ásAGNbcu?ïWuù'
"? ¿p'N`?&xԅÓü?2ÒBÓ>0Ò?"äO$´¨? ß=	å"?ï‰rAîV"?£ßºÝ=Ÿ[?iÙOduš˜?'õøì×I¹?‡-«Lô3?œ0ÛÜ ?íyD^뀹?¥ª"ÝÃ?¤Éb`¦«'?¡ø,ÅPÊ>?£¢W°¡IJ?—…†œ¯©?îäŸ÷"?¤AoÀ'a®?0Œö'ÉpI?HAþš'hÖ?¡"ô@êóò?¤Ct!#4n3FGL J0040.5-2339@UÊá`ÈWÀUoÌþ£	À:ߍ'ûÀ<ϗ'h%?Ô½
˜Æq$@,҃Åò¾?ÿ#¹€iÇÅ?ïŒp3:a¿äX­šúº¿ä77	¯¨¿¦"ãæ*',AGNbcu?ïÕÓÒDaŸ?";Ý@ÿ?G1›:3z=?mm|þ‰A?r/ãvˆÀô?'š†²¡ác?%j1Ò?—a©§gõ?G+½¡ÖT?SrnɊ?ˆ*ºËV++?–ÏRŽÖo°?î;p½—:€? Z‡0‰›¶?Ž¯H—c?€¡˜Ÿ
£?¤"³'
?ŸmðË/´n?ïY›¢?"Hœƒä?<·ÚîÝÇ-?Q—twè_?"Y¬QAæ ?"%ÜïC'3FGL J0041.9+3639@^4´A»Œ3À:+ä€G¸üÀ:»•EwÀ;÷ÇúÕô"ÀñçßÃ@bg¦'`B?ÿœ»úl?ïþÁVw¿î7à†4¿Å#»L'ö¦?¤»ùë¾ÕhAGNbll?ïò®Y¨fÇ?g7îŒiÐ.?õî¨p?(Ç›jž?Y#úͳ…<?fŁ(?œÌ?ïÇyøQý?z¯÷?QTr]°%%?XQ8_°eÜ?wíç@
ø`?wtÉ{Hn?î7ñ4Zv—?š‡I'X?ƒã3ÿØÁþ?sµ³b8êœ?§ˆºbf ?š(7$C'~?ïÏ ç?Y?vӂN >À¡¢ç˜i>݁V>ìŽ?x-£Øa?vÒoÉQ'#3FGL J0042.0+2318@^	F^‰"SÀCÂߥ¥À:‹ ²'À;Ð:‰hÊ?ØÄ·omv%@¥¥À‰d@Õݟ­ÚÄ¿âxj
K(Y¿ç<4–,8¿àn–
ÃÓ¿ïÿÄ^œÌAGNfsrq?ï"D%eÇÇ?Žô­e›òk?M%چÇI?MäÚ-%à#?‰˜þ!œî?Ž4'Ò«?í½30àà?¨³nŒ	ð?ë»iٌÁ?'! Sì1?«¶ï=8²?£/;Qd?íq %+'h?œIÑ$Šp?¢.Žbó?{0•?¦·æªvœ?"Ÿ•±ûc?ìmÁõþH‡?¥<î-?—""J…??ÄöoFÆö?¶­}lx¾?¢{·‹3FGL J0042.5+4117@^He¶™…À5‹x_.QÀ9ÛÌ`–BÍÀ;Ç6oþ•?ãˆ=ZmM¥@
kzÜÀ
@¥ŸŒLտṙaܔ¿âÛ
½Wäÿí7ž­)Ä¿âæa(9.OTHERgal?ë™ÉLJ{?ÀcÄbô"é?¼u
k?¿5¼ø?šð¢[?œÔ'Qí^6?í/ó:ƒ²?¿ëÕó}†[?¤È¾ª«P?°Í|| &?¨Er!¬Ä~?³Ô±û?«?ì²üeR9c?¢'K9ßê?¥¹¡M˧?"Ö#óQÖ'?¯*	Žž6?˜p
pA—û?ç	*ìÄ
?¼pùºí¡–?Åødã¾Ç?¼¨áüïD?½¦·Ð1…?°^qYE"3FGL J0043.5-0444@]rö@c^ÀPâŸÞW9À:‰¤f|5ÜÀ;Èà¨KäÀ
ÉlüX@
'¹Özök?ûÀÝ "šY¿ì5aËÞ!¿Òƒw³¼½¿Ð´
¤¿x¸¿Æ±
3oC/AGNbcu?ïù¬‹Åod?FtŠq=?Vt80ð´?Žˆ^­Bô?GCc<S¼?E¦ü1µ¡Þ?ïÒ;`&TÆ?zsR̅›l?BLzË´ö'?MíÙýây¹?t˜À"^þÂ?x±J¦¬kÄ?ï33¯nçk?'àgDÖ?}©«
üÛ?kÄà`Pä˜?'/OcÛê?|–í"#{?ïõ"'Î?\(/zê'>i£ÀA"ýÈ>‡F¯¾Sš?UºÇ™cßÏ?\'è³"Ò3FGL J0043.7-1117@]žYò»ÀRƒ¢ÿßHÐÀ:O".bêÀ;r²¥Z?ç÷ lÿT+@
Aï8²?ùæÀ
¿ïþÏA­Z¨?ïú˜G£Ç¿Ò±á3·¥¿×‰ùÉ/3tAGNbcu?ïõ™ÌÈí?jíáÛí~?%–€'ù5à?8~þ¡ƒF¶?R–[æÃP?je]öÎàj?í æYˆm?¼Ç˜àõ±_?–·? ;Ý?¥"êµP?±JÿÕ­¥?·‹·‰R×?î»;µ†`?Ž·6>BŒ?‰HÊum?{x‡µÛÝr?œäù´²°?‰eŸí86ì?èé.ªyï?Át¡Ý®™?¸[ٙ#0í?¶U«p;°?À-XüÄÌ?½Ûcƒ:_¯3FGL J0043.8+3425@^J:>À/0À<j'_8t¼À8¾Ž'b™À;Xó"
3¿íÓ>Bä_@žŽ5	L@[ŠI{õ¿Û¬š%8Q^¿ãʽ ßÞø¿ÚxÈՂ¿ã%NŽáã=AGNfsrq?ïûh=Ԍp?@±S«&?¸0Y	Ñ?9Ážý°¥?A3…¨=,²?@2ÞÒ.J<?ïÀê?¨7—?{ÇS•Oœ?P-~Š·2Œ?Tñ\¨únW?{€‰6h ?y˜´ßÑ ?ï?õŠ¦+—?ƒ§Vó›V?x'k•Ï×2?jCa
¹L?'ܳÅƗ6?€úbÍqŽ<?Á΅Š?ƒ±›Ú)]?ëiÃG®?°
]㬄?Ž@d"›V<?ƒ®)H"}3FGL J0045.2-3704@s`—ÿ›V2ÀSý£¿ø¨ôÀ9x/Äé©|À;êöÃ@\¿ää†Ê+@¡aÈ
þ@Wºßd¿åþóX¿ç'¨²¢eV¿å!¢qPòƒ¿ëGóëZè•AGNbcu?ïïœòì@?ez¸ŸÀØb?8w:"Y?;«ÕÄ«a?Z\÷'£A?cEY~fŒ"?栗~Û	?Æ>ʤ?Gt¦NŽò"?Q7çª$*2?"¢4»`NŸ?Ž¨?)ë%X?ï á…-á?ˆøøjµÜb?mê&ci?r˜¦Iؚ?",ÚG=­2?…+t÷‡C?ïÞ~ôÇ$?n§È¾÷ò?	1–¥œA?\NÆ?p–s9D"€?n‹¬á)ô3FGL J0045.3+2126@^CÀh ÓÀD³° F\À8Ú0òçÉÀ;Dþ`Ï6?á!€:ÍÜA@WÛ÷âû?þbw¾þX
¿â'T6@·^¿áOC¢Ê£Z¿Òøx‹›ÃÚ¿ácuxۑ"AGNbll?ïå"áÂé?d³«':@ù?4jޑšž³?.ïj6náq?gîL	Ä$?dk1¼ ?ïFH»q?'½B	¿øs?h-J¡Û?lÖwøç³?":M˜½E?Cè=»Ž?î{êc¿+ê?"ªK9U®à?Q"ò"îd?Jä'è? ìø‡lÙ?X} `Ÿ?ë™/"g¢?£òÂe¥ì?q€ìu?r"¤åy5R?ÁsŠ‰¦Z?£Ý²ÍgY3FGL J0045.7+1217@^/l?Ä;.ÀIG™¦5À9AvK¶·¸À;n T3]û?ÀŸ.—@ëáwÔ¢Ú?ÿ[@š$¿¹W)˜»ßP¿Þwa¢ÿ–E¿à%Ùºµ·Ì¿áͳiEá-AGNbll?ï½GPúr?}
¹8á†+?U}ýô•:,?WLÈ%±8e?{üøÚ]x÷?zQAï!¼?ïw6E‡¢?ŒÄù©îù¼?b:í"ûp?f¢øë{"ˆ?£è¢¶=æ?‰ÓYªñ¾?î[ÌÄÄ¥?":C3—?"€¦¡+˜?‡ãLãG? àc(4`?Š©""_Rø?ìu›áõ5?û"2H'Ã?r+$ŠY"?n[éKÙ¯?»0n¯JÄØ?ûäz"é3FGL J0046.7-8419@rñŒ¨À@gM@$³>À9Âw»ù?òÀ;¤gHäu`¿ÛÖ'/€‡@'ML @¡€mΐ¿æ"œã·0?¿æŽ8'm«¿ë!ghïؖ¿ïÿŒDÇZGAGNfsrq?ïôÎùz~—?R¼Î~­4?@øßTuÞ?ETk	±á?KË:ÁŒ
?J1Ջfñþ?ï7"W«î»?™[ÑßmŠ?r¯#øsžr?xŒÙW‡Y2?"aÌe@Ó?•øv§–ýÑ?ï'›¡¦?…ß–Lq%¼?Œ0p<+`ô?}¸Ö®4œ?‹îèےuŸ?wŸçá3¬œ?ítEç@Ê?¢èMZ+@µ?Œ¼Û?,º?ŠœÑ›Ù33?°Æ5^‰k? ã‰á_'3FGL J0047.0+5658@^•[á¨&$À"›!
À8¹R¼ev|À;\ êƲ×?×
Õ*ŒF@=ijý¤Ü@ËC =͖¿åXûRWvñ¿â4Ä¿àR+•:m¿èvK-GXQAGNbll?îþhÇ%O?ž˜™V<¢‹?z‹IâWH?|zðÁxô?™¢ÀJ§?œ'D\­ƒ,?鯦½W-Â?Æñ!<ö¾?£<LÚ¨?©•Ó#I½?Ä|â;Q?À˜J>Ë^?ílà£e»? ›'ʜš?š%™E®h?Ž¨Þ0¥|?¬k}wk?—KÕíÍ¿Á?ì"«LÝM?¦ËáH?¶æŠn?…Ĉjüv?»-¡"vz?¦ø«i¸3FGL J0047.5-2516@X`ñ7ÀUüæ?Ïù¨À9yEi–œÀ;¶T¶"¥?À7Šïuq@54wž@ZVߊ¿Œ¿âd+Xs^œ¿åFÝA¿Þëqø´1¿æ+
:¥"OTHERsbg?ïÅ3ËîWJ?€q""¨>P?N_‰yöÔÈ?SkèÅ^ˆ?yš(ٕ?~'èæ]±r?ﳂdf	?'jíÎi?b¡ð^J?zC7÷Íù•?}.ýBÌã?‰v[
±Ž?îàÕ}ñGz?P–©­§?…?Ž¯A¼?u98©¬É?™EˆêRïé?‡{Œãnå~?폖¼Ž¯?¢"CÕ5?l&AY¼?n·‡Í©M)?²¢ëÁ®?¡ì•ÚH13FGL J0047.9+5447@^›û'ÃÀ $y?ÜäÈÀ:<‹ÂAÀ;ªU‰ŸP"¿Ó"m|҅ì@.‹@š?õVtªL?îé£%o·Y¿ç²õ «†¬¿â?ñÙ
s?á0êíZr#AGNbcu?îxù¶m?°
´®rGË?B¦³ùKÔ&?IdÒM<X.?¨4C ié?°_Îâ2?îAüåL‡5?¸gcÚ3xA?q/Tiû¸?ôo¾pó?©ºG(êMU?·QÄxIkû?íCº¯©Ý¨?žõ‰\œ? 2?¯:ÓÛ?"nhìA?«'V'Q ?•‡îóßT?ïC•‰;K? 5;ž»ò?,£W rõb?HA=ô˂Ù?ž>FŸ—°É? -ï8"=3FGL J0048.0+3950@^Ž&áY.À7$_ZÙjÀ9ݏRîº]À;¥e5
ÿ¿øbf	aÀ@×)_õ³÷?þna«¿Þús&pà›¿àÇLÏLÀ¿àc¯1±Rô¿Ä30×ÁÐùAGNbll?ïö¸C+ÒÔ?R?Àî[¯¢? &a%Ó§?ìf³kH¬?PŠ­…•›ƒ?Q¥»Kò?ï˯äPy6?y"oЍK§?NÝØ‹½v?W÷ë4{C?vLR×±ìý?vÓMÞ[…?ï<Fׇ/?ƒ"š5TÓ`?€N´j¦Z??rÛþ®i˜?Oâo»í@?|:wòó?ïÜ¿'°ýu?kÿÀ!J‹>Ò}NCn6>äE ¹³
j?q›—Óðj?küä&ÌF03FGL J0048.0+2236@^z)à¤&ÀD!Ðß´0À9,ƒöš%±À;™!|QŠ6?îá¾y!ÿÚ@îþj(½¹@ª  žŠ¿Ût'冓>¿æ¥ãµ$B2¿ãíw3µ‡¿ë/EcškAGNfsrq?ïå©|l`?b,v•Z#W?R½GY«§?M6⨲Ž?`÷ýðOÉe?]ISð*T?ïºwíN¼?~¿ š?MÊvûH)º?SЉW?))ïœo?{¿á «b#?í×EðMÏ?š\ì.ä°?¢ç;ÿ"ÎG?"˜+B²%^?ŸQ_C°©›?Œ5QœÃ%?ïžàz™á?†&M{Æ]€?E
M͈ÌÐ?J"fCû8?†÷$Āûe?…Ÿ…·ü3FGL J0049.4-5401@rùm`ûHÀO6@-íyÀ:}2Ȫ(À<Çhß½j¿ÿGDAùI­@ry-hmþ@%µ\Í¿æLÝÏ\&пäcieŽ¿ßúÍì\Š¿Ö ='tËÉAGNbcu?ïÛîÂÛIƒ?–s̹6?'"Å՜$~?.e'-–?qLxc®]S?–~³­$p?ïÑà¿+?yæ:.ù?BÙµ9j(ä?L6¸Ð³[–?uÙVó%b?wâ—G'­Ô?îß,—©Ž¥?ŠHã-¡?"X"]Õ??rw@ªÇ·?™î[û@à?†"wsß?ïÝ,¡ù?hþHñêF>Õ6 {j>ä9ŽÅÐ$t?qda–âو?hù꿗¼3FGL J0049.4-4149@s[6†¥ÀRÓ@ÃÀ:–²gƹÀ<"ę¿Û;óv.Û`@­"óoMì@<zßð&¿æðÊ㓍¼¿êöÇvõֿʪ 1'%¿È9[ã¢ô"AGNbcu?ïê&1­M¸?s[ØÔ:™?gÆîÑ{?#Ñð¢›l?e•ŒzÒl?sGbn¦¸H?ï‹]«‰ö?¨HèO¹ ?S®6zþ=?k«Ÿ<:ð*?Š²ÎN_¾­?§ÒÊ íÔ?þ#üê?Œ3m9{^D?'G®æ_D$?sCìYßÁ¿?Ÿ…èÈPÀŽ?ˆÈރyæž?ï9[L±½?Ð30å÷Ý? "Ítuë?6î²·Ð+?˜»jû€Ü€?É‰–Ö3FGL J0049.7+0237@^…п "`ÀNJÀ²¤À9h"t¼À;°â`²È?'ãY,@è(©c@óËßgD¿ã,ï!¿äºjþÚ¿Ý0r‡B:¿è<IiÖ]oAGNbll?ïË÷_B]?€åŽP†§?9"a5B<??;ƒÐºÔÍå?xl
K}Q¥?€zв1ò&?ï­X.æ^?'ìV™¶?UfŠ$$?[÷
ZÒ?ý#Ãô9?Aó*(üµ?îû
¨Îó?‹…f>Ãbg?€ÎD(›žš?qÒ@	äËÓ?˜7šv˜Rv?‡.^>í¯?îöguÖü?'ä]@è?Lƒ¬c<?M†ïYø? )†"ßüˆ?'ßÕÙî,3FGL J0049.8-5737@rõœýç!ÀMÀR@>´qÀ9ҝë7òÀ;ØÌð;8¿½Q‡Ðw@‡ùZ"z@²'€Ê÷¿èà{ô-å¿åòˆá±O¿åîôŒÚD¿Ò®D$ТAGNfsrq?ïÈ-n­ÈZ?|¥&¸C?WÝIþ<ŽÅ?XIסG~ç?uñö)Œ®Ó?yD¹øad?ï¬7óƒ?‡•KÈ5¤?TlD¼2?du&?'ki'é?"JjH!«L?î­M-X+?$ïÛOé?ˆ–€_Sû?vNœi1ϕ?ž%R¼÷?‰Ì¿ügç<?ïYZFÂ
?'öjL¸pø?Inû>¾?RN
ÆQí?œ)\ßÄ|?'Òó×b›ð3FGL J0050.0-4458@rû¯_Ô{îÀR	â H¤À:NÈ>Ȓ«À<Üq…~Z¿ãP€èa—Ž@è«,¾úÒ@9Ÿ…@ò¿ç³Zh‰à¿ààêZɜŽ¿ä*NãgîÒ¿ïÿ—w«];AGNbcu?ïë;v?pyï쵋?Z~1t;€?jFßlԑF?Oš®°¡°é?Vöz½Õ?ïY'Yä‹?‰r"·¦?\¨ü¤	Ž?a˸¨Y?ˆT{Õ<?‡RB"ºÝ"?î_‰ím÷¢?"ÉR¦gþ©? Ûªª~ü?'È'§ÊÇ?'Wnì
³?'<ºYLº?ï^äbö­?Š&£îWÓø?[éQ$Uz?d±¥è΁?'se'?ˆ·ãÈ·ç<3FGL J0050.4-0449@^"¤as¸_ÀPìû_ò®ßÀ9ž±ý=­àÀ;§Ôî~:¿Ön>ڎà@'
ǾÅù@™\ÀJ]q¿á—:f®4Ü¿æ"Q¦ùT¿ä@Î>p´¿í"Ó_Å|AGNfsrq?ïœÁý­?ˆé`Eºµ–?r»ÇŸ@À?s	Îøógu?;×ñŠ9T?",ݓصâ?ï?õN Lß?œºÂ^UèÏ?lrþ&—£û?t<'/Ԕ¯?"röw#o?™ÝË6Ԑq?îm£?D*I?"ßwœ›ý?˜×Ž=k?ˆîn\/Œ\?™tìy"?ˆžª'^©T?í,†Ý¦zM?£2¿}
f?ráG#Ñ{Ç?s‹aG<6°?µm´ Ö?¢¤æ7c3FGL J0050.6-0929@^•-û¹ÀRÄ`Á
À7ï;M;À;
;…è?ÌÚ#ޒ®)@ø‡©'ö@¾ž²gÇ¿Ýè%Õ#¿âËÿóγ¿áíT<ÿK¿ádiÛ±ÖAGNBLL?ïô¸`ÇÛ?hÙ'ÙRÁ?P18(ò?
p··!#x?U¬¼æˆ¾?h·.vß8?ïÂuÅ@¼?ˆÛÝ'U?DoŠ-&u‰?N©?XÁ©E?|eS׺Ó9?ˆId`n?î‡/^ãA?–a¸.]Ôz?ƒ&"Íkì‹?z…¦i¯®ò?¢Ãe$†ÐÉ?"c¦sۘŠ?ïªø|\#W?"æx[̗Á?ÛCÿRw'?ÖLöҏ¬?…0¤÷כ?"âÚÖɵÒ3FGL J0051.0-0649@^ª`4óþÀQlÆøÀ9'Þ³íÀ;€X‹Ž>?öÛ)üþ˜Í@]‰~noõ?þôwÉe9@¿ÛÐ\ùпäñÕøO¿åwåiÑ«¿ìh­ø AGNfsrq?ï¨w¢in×?…6µ508?w«8ºò?{íç­[ÀK?töV}D?y 	TB&?ï¶âgpFÌ?nüAb?Q×»¡µ>?W¹‡_A6?€n±úœ?€"Ü	å;:?çö¹Ññ2?°yeôKÁ¹?Ä}#:¨¬?©vF/¨Á?·Oë/D?¢öóìl?ïCøPQ\?'´™ÿ;q?Xê÷ñ{?]»…~ùJÀ?–}¦v¼Î?'*ÌV®3FGL J0051.2-6241@rïj_"ÊÕÀK8X R…ßÀ8Ô¢ŠÙã6À;ÝS¨?ãiËÙìÙ@SBïòÌ?úœF__áè¿å.w†Á¿Ó3h7Kñ›¿Ì{fLTU¿Ó)ÈÐ,ÂpAGNbcu?ïÀ"®F?{é1#u?K?đ
ì(?Gì!óÎÕ?|N…¦ D?zÏÔ:=š?v²?ŠÚÉ<ÃW×?_E—[è?j¬öT0JÇ?†1ì²(Ð?‡F'i¤"ú?íQ²£éJ? }3÷=?šk¹x™Ö©?‹>ûðÂ3?­¯)t€?™ê/¼ëk¹?êßrê$g?¯ˆŽ¬
…?j¿pi]?ugÞ[ï?ć8¬º?¯w¦ï$×<3FGL J0054.8-2455@aÐØ`fÀUêeà.©aÀ9G±CÝ¥À;Ph¯ìÂ6?ÛgÓ`¸@ÕÄÉH3?ürå?µL¨?íš®t>Ž¿Ýb=ºd¿Ó<ؘ£Ù¿àtuȯAGNbll?äe(wZš¼?×	3ö1a?OTõ*î…É?Xþ*ªX?×&–µSE?×1qP?ínŸáV. ?Ã×íöJ4"?p÷[¸O¡G?¸AÇM¹n?³{‹9ɔà?Ãz¯åߧˆ?ëð.³»ˆ7?²žEþo'?"õšx›J?…ÈzÕ–`?»¾Lû…—j?²+k#5À–?ç6ˆ¹4
?¸(ùâP?|EŒ+-Í(?€]8®~?Ñ!Ø\ë.È?¸íjÐË3FGL J0055.2-1213@_ ©?)
»ÀRÄÿ¿ÓÀÀ:xHG—nFÀ;ö
>¬ãù¿àÓ|¶¬F@ìŸf7A‹@,€0¥¿á †N
!¿çÖ´ñӆ>¿äü—öV^¿ÛºßáÛíAGNbcu?ïøÅcúk?U‹ùÔo]q?3Ý·="?(7Aýó?ID_eÕ?UAæì§ø?ïÌ:t©×?'	Œcԋ}?Dµ"'àÃu?Q&.ï³?wLFSNü?Ïf$W?ïCt×øH?Ï"o׉?{|?ÌP¾?p¨rYpÀr?²U
âÀ€?{žgŽÊÄ~?ïÁ¦•Ë?v"ÊI€`b?Ðý¯.z?V·ûq£?JQ2¼%?v‰ww·Û3FGL J0056.3-2116@`½ë¿×ÀU
€!"À9•ÄÿxñƒÀ;vÖ
c0Q?àÙo@`Ö#7½‡?üí~@!Ù? ïÃ
J/¿ÒºJ†-x¿ÛÅð Í§¿Ù×RH'ÖAGNbll?ïêh×ÕÛà?†FÄH?=Z\c;RË?B
®@d?aëܝ¼³ ?†€Æ¦tFõ?ïAÛg;žK?¤"¬ìœlh?S'ëc'Ò¨?ZÎ'ØdÃ?–ŒdbT	Z?¤<Nêi¥?îÙPq+
?"x…‡·ƒ?‡j/nj6?{áõîð‹?™ Ú#iSg?'YGx¤p?탊Ùþ"?Ÿ6·)ó¶:?aÑÝÒÇ?d<è8A?³UOqzÏ?ŸV@:Œ"3FGL J0056.3-0935@_½^	ÀRSÍ$áÀ9ÁÕùµcÀ;|Fûg¿³Õ¥½@8@7s'À?ü¤À Áìt?ìÏ96Ç+¿Þ$ÖxQ¿Úç0‹c ¿Â^P»HAGNbll?ïô'Ò?RÙ¢éìã?.—ül á?1·ÑƑMã?TõÞbÊÅ?Pù1­?ïÉì…¥Ý?{5Î%bU?EbsÐ!Z?P¤…"¯?x]nÿ¬ì?xɘ"00Á?ïâє¿¨?†ZÊÍ¿ª×?ƒ¦6r<Iã?u±¿ä…Š™?'Њ"Iåù?õõá$+æ?î¬ÑÍ3ýñ?˜'çMw;J?-µ5{7ÍA?<:)tÐø?¥-÷Dé4?˜oDaQfÌ3FGL J0057.9-0542@_ÖNaŒâÒÀQ!ŽèӔÀ:43#Bû'À;¶Ï†»p"¿ïzI²‡@,
{®÷û@R²à£¿à¼‰ô
(x¿æÒå•Ò¿å_ï˟J¿æ¤´ïz;AGNfsrq?ïR+argD?—#‡›§P?]ŠL¥?_…÷Ö?"éK1q2¢?–tÕ/3?ïªcñ–'?Š)"CÄCé?W‰¨ñÄÒ?o×~·0¦¦?'uûN|=î?"Ó#
퉙?íWë¼±"ð?Hž"6–?µ@BKð'?)›IHâ,?«¦¤Çج?"´ÐÜH?îqoAìYw?—a¹ÍìÇ?DÈen'æ®?F5Íˉô?¨•êK€Ý?—=ëÀéú3FGL J0058.0-3233@r	€bïÀU¿ÖDEÀ9C'5ÏÆÀ;€Æ'—¾?ï+I˜¶€ì@¢Ž>F·Ÿ@w~?ËòÝ¿Ü«#ñ2¿ÞšMìût¿ãX^v‹€/¿âm+©û~AGNbll?ï¼:mâÏ?"Aþ+Ü3?UókÀ±Æ8?\'Q÷Ð×?|eîb' ?"âSÊ??í¤ü
H9d?»ÛJ5DžÅ?{i¸°.?Ù[(fŸ?±&)r©Ü?»
¯Ë¥jù?í¬îh6ZÖ?Ÿî+…Šâµ?š»7ød"Š?Œ0Ë4P1ï?§Ó}€hY?™Ë†ÜÀ`?êSÀIŽ?²b™Ä/Tõ?—úÛúš?"ijçC:?ÿ[w(F?±XF¬Ù3FGL J0058.3+3315@_%þKZÀ=•2¯ÈÀ9ή"i›À;й!õN?ÑÞüûÛO@ç0+kéˆ@B"@Îé¿æTgê䩧¿â.ñ°¿æ[š6nô¿íËLŽ'JAGNfsrq?﷗n`Ô?{j-vM²?xø¥°}ß?vKµ	ð
?fxzSÊý.?eî!d?H½Bç?…£‹'E?`‰Øíóˆw?d3Òß—'?"5·•2d"?'šN9<-?íݞkenþ?›‹Œ–o%'?¥çêÅþÑ?•¼°'•ú?˜|^oÆ"Î?…®"S‰ª;?ïu5ªGzZ?‡ýúΰ¢?d|™"…1?a£}ŸxgÀ?"o	@I?…¡žÅI3FGL J0059.0-7242e@râR€jôkÀF5W¿ÚvÀ7îjCj¹À:ô‹…à_?í]ñg¶È@AT;9½@đ #a¿ÛÆ2x'É¿ä•×m9¿>¿ävôô3C#¿è"äÞ¼csOTHERGAL?â"g£y?ə»mË?¶
ã "¢-?µ'0ˆc¿?ÕVwýÀƒ?ÈXèÖ©¸?ÛkâÌ-`?Í>/øOúg?Õë`£?ʇóže?ÍQ·tOj ?Â74"öL?ã´%چ–Š?³¹îÛ?³.§Iò?¦fŒÁE^a?ϵg>[è?¯æ­$½Á?ÈÒLÀYZf?³²-:,Òÿ?Ñb'xQpü?¾ƒW/<Gz?á$Àðè?¾Áªªé3FGL J0059.1-5701@rÍÆøÀN	T9À9~@¡°À;ÉS¿šµ?î°–7@¨•žÃû@îpnö¿ÞTíPo¿ç•>&þ¿ëH_TÉ¿ïÿåώY[AGNbcu?ïÉìÈ-?pÛ¯÷?ekB‰?ht¹Îpq?pTl˜qGâ?}]­®Ì6?éB°þx™?Á™
* b?·Õ+¶j«?´4	Tj¥?¿0¾Á¡?¶Ÿ8±ã^?íU«½S÷¡?¡q<GÛ)?¦ !ªò!O?—H±œ¾‡v?¤"Îd¦?"J `›©?ã¼µˆ.M{?»þËæ‰"?͵^Nv"M?¶Ø¤ò9Ä?ÃWːÐEÊ?´aðÑ´¾3FGL J0059.2-0152@_߂¡/ÀP+á .QÀ:k+D´À;½¦læ³(¿Ô·Qª0"q@ï9}$C?ûÍ[ d¹é¿Øµ{!‰g¿ë´kÏhç?»¹=ìÓ0¿Í²w°}þAGNbll?ï¡Lû)?­Of3£¤?'óàxYÐ?_ʶš?‡‹»'—Äò?©ñVåµ?ïÊå'Y£ž?{'™bAç:?D·Ê½—m?O-'žm–~?wö=û‹ž8?yŽÖy2,Ý?î³±éè*v?š›¹+rÓ?…·±õsA¨?wkžÕ±?ž­éÈAi?ˆí	»¹Ih?ï$9e@v?"ü3xŽT?>þ§?‹#õ¸	?œÐx´Vî¤?"ûRÕ ,I3FGL J0059.6+0003@_ÙØà†8ÀO_Ï¿ÆT
À:J'ÇÅ&À;ϸé?á÷÷ßA'@¢éCÐå5@ß&_3i¿ãÓÕ!&Ž¿æ5h¡Bõ¿çÀµQRzn¿ìŠðð~¿AGNfsrq?ïwÆi·¹?Œӝ‰"?w°¡pž?t®¼$O}ò?†µ6ÙŽ?‡èn =<?îóX™—¬Ø?ž¢ùˆ­?zúŽš ¨Ä?W•BaîK?šÖI&b:¶?™-Íóˆ€~?íƒ*Cý?%ٔe4?¡;8
î¸v?Œüف`rE?¦"Æ_mÀ?"Åæ1s±?ëˆCÖ;è?¥ù‹ ¶¢? Mû¾È?EÓ¤Ø)?»™]ãn¼°?¤€.8ŸÃÌ3FGL J0100.2+0745@_°4?¢­?ÀK…à
—3À8«sp:$¿À;
{¬HÈÇ?óîCÍ_CÝ@«wènê?ü¾ÌßAC—¿ÂhÍÿ|Í[¿Ó¾Å4ts<¿Øw=N?(¿ÛþNuÀÒAGNbll?ïà'î?sæØØÞ.?A_®†Ã¶?EñÀÚ©Ž<?kŒ§	I`æ?raq.ot?ﮈ(ŽJ?ƒêÁ=4º?Tr®<ý¹$?[㞔lü"?Ï§n<µþ?'\D\ò¿?ëä'Yü4š?«9/Ú·c?§pŒ, W?—Йó@át?µ#§/ ?¥):å׶ö?ëîq?Á¦?¨¯Fþ¿?u´éÔa®f?v—Q¶D`U?¿1'd¬±?¨®Õ˜ïe3FGL J0101.0-6422@rÓ[ߏG0ÀJ\ŒSâÖÀ9õ[aO¦À;Ê~ÀÐ?H?þÃ	õ¢.@
~×ÌZ6@FÂ5D/…¿Õ€ÉÈ¥9¥¿Û'hÉþÅ¿çM‹È>H¿î+
Ö
áPSRPSR?'£ä.Û!?"t|õ
ö?ï~ÿ@ן?'Ÿ²'¿ÕF?{8¶[6zž?…¼é©7š×?®;Ý>é?´²c½Z
?çǝ÷¢ì]?Ä×.^Ä?ÉRÜä"H?Á^/±ý
^?¨{»á¦?špaÒi?ìlªZí?¥üO>˜?³Ÿœ¼UM?ž½í¾g0|?»†›ÙÝ$I?©H0¸{…?êWd^ÿÔ#?°[¶ä'ÂÒ?±¾A.$:™?¦x5ÁôÈ3FGL J0102.3+4217@_Eð¡¾+IÀ4‰xmžiÀ9SDñ¡˜À;Â"³‰.è?éSGà¿Gÿ@š€Ê?Õ@ˆˆŸÌ8¨¿æÔŸÚrÊ¿èžr!c/®¿ë…܇n¸‰¿ïü-êì>úAGNfsrq?ïâ
DºmÌ?¥6
°‰D?išIpå?¥8Wc–??AbŠá#ù?C¹ð…Þ?íí€[†ü{?¯ÐuÅÉ°b?–À£X2°?šQ瑹Ýð?¥Ç¨›w,í?§Ó{D¥µ?îïǹ
¦?Šb‰p&2«?'44çÄ?ƒœ˜9±2?Žéäv.á?{àÀD*®1?ìÀ^‰¤~?©åé›ýõÇ?©'­ÖŽ1ú?Ÿræ•êûÀ?ªÒi˜W†<?£S'ƒÃC3FGL J0102.8+4840@_7ƒ]íñáÀ,Oö¿ž(À8ÏϚ¦ãÀ;MIðäÚ
?úÝÙìD@­AÂ<@œuhâÿã?‹þrى¿Û®Ó朂¿å‡)yù\¿ê-s>¢8`PSRPSR?¶î"Ò,1Í?°ºET‡©?éÎþÇ©'?ÁØÍYú¾³?º «7–'?¹jäÛ#?Ì¥WêÆH?Å7ìŠêè¸?ဆËIɚ?Ç/²&܇º?ÍXŒè½L?À@%,ðBÊ?Ô´"œX+,?³ñ|~EQ?àw"QΠÐ?¶nܙ‡"\?ĸǀ&i?«mø)#Ï´?Ì3ÈäÝ?¯»
]ÍR?ã{Bë‰$Q?¸™$¯G?ÅõÞ‰ß?°™Öd®}]3FGL J0102.8+5825@_B€®IÀ¨!ßβ*À7‹dBSbÀ:ú3ºA¯Î?ú‡Çßþù@;ºjŸ†@²,±¹Ëé¿ÝƬ_¢…"¿ãÔ"‰Sw¿åЭh>¾é¿æÙ¾«T‹AGNfsrq?ïo9~úx?Š°™î²½?l7œœm?n;-Ðûón?
'"FÃ?ˆÁ°ýÂ\?î~µ¿{ús?µà>A£ì?sìÐݘ'?‰'[{´ÚÍ?¥—	ìeÀ?´ÐϜ±Ð?ìFñÕCz"?¥ä=ð;Š?¨tuÜ»ã?™Hçjÿm,?±Ž6g†¨î?ŸµvY™û?ïòÅ`g?hd˜ot>ó"aŸè-??N1h¿ý?[ª$j¿Ž"?hž÷ê~M3FGL J0103.4+5336@_/0¾
í)À"mµ'm,À9š<Z#bÀ;•µav<¿õr`''èu@®µ©D²@Oë L'(¿à…Œ¿âõ¬¸}¿ßµë–³Ø'¿Ô=ڟ%þAGNbll?î½­¼ñ"¶?ŸKº£è®?bº2ã×9‰?`×£ÇQƒ¦?¢ùª@ô?žšlˆY?îálàK?§©ù¥¤Q?kýW'y3?v=Ç"äã? 0.IhÓÄ?¥?Xe'Ó?íõ0ŸšK?•*`Nÿ-Ò?"'+ãCO³?™'Ngù?¦kà¼"p?nqKñ?H®ò?äìðh,?š>¡ Ã;?N9£XF?ù]ï2£?ßšYTíc3FGL J0103.7+1323@_âx £
·ÀH¯8à^*À:-m\ú¬ÚÀ;ËVN?ì~fº–Œ@º"kì­?ÿ½'ÓY¿èGr°K¸?––á"–5È¿×Q\`uƒ¿è?iÔÉúAGNbcu?ï¤<¸ÿâ?Œ/,6<Œt?nDò[ÿ¦æ?uy²i+n¸?~Ïhu€;2?…ÃÙNKõ?îL^'œ×Q?¤DIì.eˆ?ˆ.úm—°?Šá¢Éj®<?¥.^êÌÃÈ? ©(®ä?î
î(ßÇ?Ÿ@'Ž˜í?š®d3<?ðyî‹W?¢FÆMÈe'?•_4ќ?í5­'=Zí?£¼A²XI÷? §™½|äR?–µ`þ²ãw?«ý­lú?žk^~›Ûü3FGL J0105.1-2415@eZ`˜ÀUréÅ+À9jÑáÃôÀ;Üó…ô¡?뀾iW@@(4'@Ý砍©¡¿åË,AZ¿è'þO{¾<¿èåx.(Ì¿èΆ¢éE÷AGNfsrq?ïççRÎ}?~Æ)õZ6*?Iɑђl!?lnBä›öi?a¦ImÌèÖ?uvðŠ=Ú?î9rzÏj?·ŽÞˍS?qáâR%?ƒ'7Ü´?ªEœ¸Å£?¶»mP³r~?î>ã+?¤-"|×?†
·•?wꋾ	|Ô?¨Ûd£è
½?£Ös£·x?í¶·Ër_?§,:±ãw?‡'ñqÅÆ?"	ïÏüná?®°ìh'?¦pƒwš3FGL J0105.3+3928@_va€M˜9À7R_>SùÀ9î㾀ٯÀ;Þ
,8m/?Ó,×(ñ:ë@¼e$@›|ßy¢®¿æO¶{ý|m¿ç´2°	%K¿Úµ†HÂb¿ì@÷33™AGNbll?ïâév .?p+ë›Ý›ê?MÊv2…´?V?´øÊUz?e£ìS0~l?i¯ÊGŒæ?ï3	í¬	?"eÀ'^«P?vI•MÌÏ?tó#…¯é?"hî×|Í?'5úÆ~Ü?î§ÕY!J?"Dz	šÛd?'NáŠîZ?‡[ø"™€W?˜·HúQ(‰?‹iå%ŒÖ¶?îˁFË?"á"Uéö4?n'Hw"aé?jH˜Ð.ŸI?¡_ÇõÝ;?"4gøY¶3FGL J0106.5+4855@_^́'²ÌÀ+¾øßzN{À8®=Ç᫁À;Sà0Vßá@Úi=DY@
֛©"8‡?÷T™"öÊL?èÃQ¿Ù(…ÈßàÙ¿áêe¿ïá¼hÚ·PSRPSR?rN5?ƒ1*V À?ï×½2, ?¥€iւ™½?š±'5·¶T?¤oçkMœ?_Çë1çF?p­4G([?îHÇmû‰?­êkÈeÜ ?ª€D/'"?­Œ酷a?¡m;Yx*w?"¸;<ÈN¾?ì§%âŽY?¤jÑò'P"?¶¤)$/x?¡Hÿ'XŠ?'ã–r®?~—€óú?îÊk±•ä?¥˜.#z?©Zs¨B½¥?£o4ÕÖÇ+3FGL J0107.0-1208@a.T2TçÀR¤• Õ`À:l,µÿ+À;äkŽÄS'¿¢—z\Få³@åN`¶#=@qŸš´¿æK£ê«Z¿à>'$e™¿ÝVÎ:WŒ¿ê±K}"÷AGNbcu?ïSpYuO?""¨î×1F?}[,4 ›á?€e¥b^9?ŒvSˆ[ì?ŽÍPÓ6—Ñ?îa,?Łf?«tv`ñ¤?…Å:±(9œ?ŽËæÅ7?¤{íW]Û6?§ˆÏEÍö?ì¨Ó®õgG?¡ÍÃŽÁs?©ªÙՌà.?–Úê|ëXó?«Çë;«f?•»OGw
?ìWÄçÍ?¨¨Æ<«q?‰0ñ(ª?ƒË<—"
?¼w#¾¦<?§õ|'F˜«3FGL J0108.5-0035@`Ž2ßP]ÀO"!ÀD(NÀ:_-p{"À;ÍaÐÕp	?ç*Î$20Ì@$È´º1@&H «L¿à3×m5¿âÆïD4Ò	¿êÃPċ¿ïÿLˆ¼ AGNfsrq?í|}hüÑ>?°2`Ó?¬6uiÿ'å?­d½œ{L?˜hf²K?—høۜat?ëHϚI¡?¼¹F¡›—–?®Êࠁ?«øäQp´?¶³½«Z¿?³¤4Œ°&N?ês³{Ä?©'8}Ưý?¹†J5û"?¢i+W­T0?²Üò)NJ?šUÏèÔ?ä@>{à¬?¶Éò£?Ç·úxÐJ÷?²Ÿ…ßm¬?ÅӍ@2Y?­x'"3FGL J0108.7+0134@`{Ãá`xÀN	@¢CÀ7yÚh–ÂOÀ;Ù}µ7…?øn$Ù(OÕ@kä)µ°ü@Ÿå]½Jy¿â ÞÀŒš¿æ¶­ôøîq¿åe³™ÜÚ¿ê+\üŸBAGNfsrq?ïèc‰a[Ÿ?_mU5"{?ZåçýfÚ?XÀ?
°¨K?TSÔUK[G?Q11ó"ó?ïÈÕȱ?{Aç:§?IɉxämJ?\ÊXçÁ?x\LìŠîã?x"jô´H?îŸÛ'+Ž"?"@šGn?–óÁé£ae?Ó>ƒb?•ËÐêÎ,?‰]uÃô\?ïy…L×>?"öm}?;˜åm[?K-wq€õ?a«Áÿb?"á–IF:n3FGL J0109.1+1816@`çßã*ÀF3=?üoRÀ9ÌjNRsjÀ;¸a†,ÕK¿â@2,…Ú@
§Ü"@k@Q–ߪõâ¿âÇ6cݿׯÛ[A*~¿âðÄQOû¿ÓÔèÍçÝ}AGNbll?íD©£C¢?¶'x_e*×?]J"¶Uã?dÉB¥Âw?² °¢£	Ž?¶d8—‹Ô?\'Õ?'aìڋ¬?]qìøav²?gïú5».?‹*ë<ræ?­	¨Ä¸ò?íx›æRí?Ÿ­–<ZK?"üï%ˆ°?"/±BFó ?­ø7§ˆä?™´¾#Eۈ?îÌé±7À_?"×¼¥Œ.?P.6kí"®?SCÞÉy?¢¯ó9$'?"¸…q™¤î3FGL J0109.8+6132@_H?Ffí¿óååÀ
̜À7³Ä UàÝÀ;TáÙ¤?ûÊÉĕF@µ|Ï'@'X³ö<2¿ãáÕRàÖ"¿ç?ÄEa*Š¿ëö•¿è¯ürŠi®AGNfsrq?ïPïm­,?•‡vtµ‰€?OÁ~\u?'³‰Üé©?vIwO·•I?~oéñø5?ãp!©è\/?Öߺh¤ðÁ?˜«£Ó0ß?¯É*ò®D?מññò"?Ös8ixä?ìü;ßæø?£€<6r5?¥|ÞpmR?—õsÕö?ª¿c' ‡?šY'0?ïéô{iî?s_ÙÔ»gŠ?úN7?2Ù†&çl?e#´ƒ¡¸¢?s"ègîðâ3FGL J0109.9-4020@qÿ4?¢­?ÀS¿ä†þÀ:]Y#‡Ä…À;ÇOr.Å¿ÿô
]ᇚ@
~	æ]Â~?û£l`üD4¿îë]£–"ú?ï¾âá-¤J¿æÏÊ|ª9i¿ÉX­*ÅüNAGNbll?ïÔ3'8(è?|"~Ÿ|²?AÏ,¬šÒh?E'iœ¸Ú?s¬YNX1¸?{\Kòqh?ïÃÂ=­Õí?Q0_'$?JèV…"¸!?b®U`?zÁÖXbrÜ?€\÷[?Ëú£?Œµ°>?—Ã1?zy?}ìQŸ_ÄH?œàèáÏ?…BmzX?ïÛޛÊøE?yė¾ÅûØ?%ú"Æl0?APÕNƒ)	?q`Ý|S"Î?y¨ç›Þr`3FGL J0110.2+6806@_,‰a=1º@;N¿«§
À8´¿%DÀ;´öí1Ç¿ñÒف;)@Æp÷cú?ÿڑÿFq©¿Þª¯ iú¿âq«h#*¿ßíž
¿Öì,39¾=AGNbll?ì^…ŠÇ)?¶ŽR˜±}?€ë¯À"þË?zÞ/5'ñ?ºî]±ÂÎß?¶ »h³µ?éñô֟3?ȍâYcš¤?‹ÁÒxU­Z?•>
"d›?Æ}£ (_?Ç[_²=#ˆ?éfú?«®;[böæ?§ˆÎ€r'W?"A糎ær?ÂbæÍÃ?§¾P
?ë;¿ë?³hrÐ,›?^-²=Ø¢?kߜnXŽ?Á¾µœEK×?²ã,O3FGL J0110.9-1254@a¶êá‹ÀRÄqýÌIÀ:pµÈ¤I À;Ó	¹½&¿ìÒÏbJÅC@ȍ¸dàÕ?þÍÉ¿|,K?Ú#pqpõO¿ÚÁÜÚ$¿ê30ïꑷ?ÊY1y´™AGNbll?ïÀÅ~m.Á?Š.'N½Œ—?j&þle¨¢?pTs'U?r‰Á"5ÊÛ?ˆ|b|‡H?ï¼Ð÷?{ þ™?Fr,ИË?R¹Ö/¯uŠ?9I¹cq'?ŽË9ŸzF ?ítjœyX^?Ÿ‡Rœ¢T?£¢&–׆t?˜¿µ½ÀF-?¥/¡'óÇ?6("ªr~?ï$»W6)C?˜ø[ÄhÄ?4EVúÔ:?Iðeeøi?›½O‡7?—þñé?3FGL J0111.5+0535@`ƒ'ßüTzÀLvÆÀCQŽÀ:"#bۗkÀ;áž*øÒ¿Ï@h¡DB@»»+9¿"?þ«®>Â2•?츝ü]fÁ¿ÙqÃÇj=¿ËåòFÈ«¿â(4æezAGNbll?ïø»ìeö÷?PK™Hy˜_?'mtÎæØ?*¦sí°œ?GNó
ðjs?L߅J¦ïÆ?ïÀ³TÔ]\?€r3ü?KÈ8Ì¢û¯?RP7…r?|-N|<ò?}ÓCu"r?ïQì³?ˆìô¹1d7?…òä¤4r?x•²›²?"'ã{òÏ~?ƒkJÍP?ï*ՀÙôê?'`5{~‡–?>°îP*ږ?D,~µù=<?š*Œ+€·R?'3H3FGL J0112.1+2245@`$›«–òÀCîŸóOîÀ7FëÝ3L^À:£!
;Ã%?ø>§UCÿ3@Å~öU1?ýøã
Hٿ؜t/ó¿àäJ\Å}οáC€»Û¿ã´¼~å§ÿAGNBLL?ïæ¹ p¾?j½†'‰¬'?%¤RO2$?*"òøjOj?gìšjNÐ?j",©^Ww?ヒÒÊ9?{,£ÃJÉ;?LšÜwò$?S®zgýþ?}' Käõ?x³ùËüw?ìhíu´$?©k÷	Ž0Q? ``ÉŠ ?"&0Ás?·$ˆLm™Ô?¥"N£L>h?ï@ÂTöp?›ñ'þ~áx?@Gý"L?Pãigày?ž³muxŽ?›»FA56Ö3FGL J0112.8+3207@`)?)
»À>†§ ÃY‡À7ùpQ¡³DÀ;]*Ãøèµ?ç Ü ›×@räOOt@æšà@œþ¿ã|Tò+¿å{{°iX£¿æŽ;@Œ¦Ü¿å±ÿaýÿAGNfsrq?ïԉ,eÆß?¨ÚÉ}Ÿ,?lFöÔ"ˆ?¨((¨6'v?^_¹ŒM?\-֔O­(?ïÇóq§?y*6ž²0?JÎÍÕ4^š?Tµ5¯ó?x¬£: Ÿû?vn9^fëD?îÅ1Äæ?'éùÀ§ãŽ?ˆ`$
I;?'`'?›)µwºú+?Œs›ÜWÕ?ï÷æ~.ß?[èå6Í ð>á©êñ™]¿>ø'æŸêŸà?P¯Íáð?[Ý{"ͬü3FGL J0113.0-3554@qJ@WÀTLŸëÃ2À: W À<¾ne8i¿êøü^=@´½uÁÎ@ÈŠ>ˆ¿äGÃ*.C¿äódfº|Ç¿ïv­×û:Z?åeä J…,AGNfsrq?ïü:ðL?DZ{×îâì?$C±'ÊZX?/á¿yŸ.?4§$¶Zy??&ƒÙ?ùm?ï»CªÛ‹?ŠÛ%ˆu¾†?BëHz?P´£)H³?€`Á–Œy?‰äènҁë?ï·XG?õèZXû!?'"AÅ ?~Tlþ+]?"Ôt—I?ŠC £Ó0ù?ï÷{_èæ?[¸ß'QÍ>ˀ‰æÿª>òØsVÜ ?Pûëq¾a?[
Óq=þ3FGL J0113.4+4948@_¥>¢ŒÀ)Í*Ž:ÁÀ9I݂&¶MÀ;ŒÚF2y?–ªnxåŒ:@æì·£ÅÂ@dŽÀ!ß¿ã¦oÓ¢~ð¿æeí;›ü9¿ââëYͿ൮#O¡AGNfsrq?îÙ+ôHÚ?¡Ã¼\Ør?poXÞÁ³?pà)yË? _cãOð? ¬v/&ª€?îæóu¾K?§Äsž—$ö?úàB‹G]?4ä*?š$!&ú2¹?¢Ó* »1¦?íFd–üwö? ¡U ès?šÆÝ\Žì'?ˆ±¡öQO?®6Gáñ
ƒ?™.Ïöl?í(üÜõ¾?¢'LÏÂ'?x¸?¸=?užÁì¯Ï?µ4D÷ւ?¡Òj°V!ò3FGL J0114.8+1326@`tÿ´€¦ÀH…>ÏuÀ8õ¾smµæÀ;oU"‡"¿ü¸0ÆFuÛ@wFwÉM@žL?ž¦t¿×dÄ9Lʿ怲u¾æ¿Ýe­›{"l¿ØtiD£YGAGNbll?ïü¦{€i?=}Uc	Ï?[Ù·¬g>þ+5bÍÓ?8Ë\ÅÏè?<ؙ<WÇÊ?ïÈäD®È?yòV*L]?FºOîÁ?P?Nˆò?x¶v_Ø£e?xêj')­?ï!^ôÞA?‰`®_NÖ?~[÷‡"?uË͏ơÖ?"=ZÁâoC?…¶JûÔz?ïÙ/Ç~ñ?ra5=òØ>È(¦öyJN>ßI1æÑ?se,·Ð?r_Kž½ð{3FGL J0115.7+0356@`Ѿ ºKÀM0¶ßû}ºÀ9	ÓöeÀ;xÃkúúÞ?³©ûæ"°Å@[Î\ïÅ@ñÌ )–&¿ÙÊ.Ýc¿æ€=Ÿj5¿Û°üýl&ð¿âþ3¼×?AGNbll?ïŸÂUƒ,?"úÁyïŽÎ?V~^PN­?Y		žü?HNÞÕ*Ø?"k"š(½ž?ïK1Àx?§Ú$åvÿ?r1Ÿtbq?‡
£§Á@?š
1êçjþ?¤¥À$>îO?ín{+«÷q? |÷™±…?•¿oT8—?…Ê(«h†c?®8•›$=e?šÅeâۜ?ë™ÂQ˜¯1?©úšï?k	›.G^?l%уõ+?Á,ÐLäî?©Ó¦È:o3FGL J0115.8+2519@`;[ߏG0ÀB›dÜY2À9ç
¶<À;aìNrSÚ?á«ÊžŸ=@Ù»$Ù©)?ÿÊW!O!¿åޛâi¿às݅+Îe¿ß>ß)×Ðó¿ÔkêÒÏνAGNbll?ïèà‡Ú‰â?eA±E‹¾?5–ÄÅ`€?0R'uÚ¢?dlŸŒÊ9?d¦íØÓ!"?ï™?n,ú/?…ݘìä5?Vp|'½?X×aM?©$?†âäo¼•?"Bd7QÆ?îÿ©L«4
?'–å!š?"ؔ²I`?yë²% kÒ?•ýê @Z;?‰øk›À$?î6t¼È¤?˜¶#æH?a©ÜCLJR?ej¿¾š-ÿ?­úïþ±/?—ÃÊEw"3FGL J0116.0-1134@btÀœ<âÀRZ?ßéàÀ8ê`ão¦À;¬\ê½?êë5·¶©å@®!èÝúr@ÀPÀ6çH¿Þ.ëlcð¿ç´Ak	¿æ¡g"âöZ¿èRàÄjAAGNfsrq?ïà͞ˆe?¨¨:'?5è/–Njì?0¼àF{?lu["˜Î¦?¨'¹ÈԒ?ïÐÂþOoÏ?zã÷—oŽ?A35#²§£?Kj–`0Fh?ux3ÑÃé?xÕÒçÞT?î´o8í!?H<Ô~{!?‰(Œç ?'®dõëÐ?š­ŠNÈ.?…õëFžüj?ï삖¬Ò?h¶ m~2Ò>ýç"Û=óù?
e›$Å?cAšI»².?h¡šöYþj3FGL J0116.2-2744@k–PÉSœÀUM`#UÀ:jâÌéRÀ;ñ[dR?¡ZT¤
ûu@
—&`çÌX@.ÿ—ÐA?éÄ×Ä]Σ¿ÞɌráì;¿äƒT¸þL¿Ó¦ýÇãÑCAGNbcu?ï—Mí"-?—2xdB÷?^¼¯aL?dIœø⃨?†U9¥H{?–¿ÿ*Õn¥?ï|Vö|Ø?™ò×L'ÛM?Q¯#cÕ3E?[Éð
%¸•?Ž´]ôOR'?™'{Yö?î'¿þz£?•W+®yZ?–JdÓ-×¹?†aå‰&>?¢^Ýfiö?M©V­y?îszRµÀU?Ÿô"M¤'â?c::š¶‹h?oæh|E?§"·*ø'ö?žú!âtÁõ3FGL J0116.3-6153@rœû`(^ÄÀK~'Éä»À:ѵiÙ¸À;å€~?¡¿©M -Ì@¹"x˜B,?ÿd¿9Ú¿ÝCbB"#¿ådá¸['¿áuÎw¶‰®?"%µy҇AGNbll?ïÞ1Zƒ™?sñ[r}o?4Ü7ªE?;éM…Ã0?o3#6±	?s+qæîšÓ?ïÃU.ÍÊ?{©«?IkK`$?Q¥Ùí:ÿa?{Gó_-b?ycA"`£1?ï=¦N\?…Ü[PÔ÷±?"2¥rˆN?sׄj•þë?•ßC㄰i?€ˆÒ>±Â¶?õ"'?w`e^ÝE? &9¸"?2ÿTÏô´K?‰])¶ÄûC?aBW{½3FGL J0117.8-2113@e:Œ¿+#šÀTdŽà3·À9Is§—‰À;>e§#ÅØ?æj³Æ§ªæ@Ÿæ:@"Áÿê0‹?ÈÞ÷5šÛ¿çpws¡YÏ¿ã¥yéï¿çKÓ µ'AGNfsrq?ïÝKtÁ Z?€
Áïÿ«S?PÚhaF?S灚tÔQ?jGˆ¯+uÚ?)!Ixñ?ïA	±5yù?¤'¨<î:?_G#­s*å?dF¬$ïã?•êWžyŽ?£·z=Õ-µ?î'Oy£ä?–ðW{xa?'úÜ%Wð"?ny4½2¼?¤šS"It?"«@ü•Ø?èò[©é¯?±ç Vuí>?€™;5	?x{qÊ°K§?Ë,ý¥	Bõ?±íé?Q.ï3FGL J0118.8-2142@e¬Ø'tÀTorßñl¿À8HK"bаÀ;ô3C#k?ûÿaw>Oò@½ßtWj@š*ôw¿â¾¯CAk¿ä֛:…¿äá§fz¢!¿éþœJwÈAGNfsrq?îË8änÃ?±f´³Ó
T?jèuÝ}_•?mË5fOa?¡ê[;ùˆ?±K|Ѫå?ï+ÊÖg5F?§Óøu֙?Wý‹ŸL?gOÎ)w?™Ìy'^q?§txFa?ìÞhV)?§®{ȗdÕ?®sÅz)­? ¯¯ýþœ?°E†~9å?Ÿ"¨6"â?í­¼\ˆ?ª
¶ú¢-?k*J ì¤?uÍ'÷z?±º'Ê5ºß?©s%kœ{Ž3FGL J0118.9-1457@cl O*àÀSt`$-À:Q¹  À;Ȭ¶¬Ï׿º[Ï@'âã@
]7Ÿ©~?ü"Ëÿrfz?ïŠeöÔÞ¿á†áÖÃ-¿ÞœÎ¤µ¤¿²8}4‰¢AGNbll?ﶊ>ü¦¡?'ïb ?7>€È?6¿Œ%×Ó2?¤†LÕ×¥?íÔmã^A?ïÆ?:ã2p?€kL«ˆ?D²8S5(?Sé§6Yî?zJ"#"?}褤—Ù?î¹mUKӐ?ˆC¹XQ?‰ê@'ô´?uO"üLÐ'?›Ý53Ñ?ƒiaJò?î"Iª^1?žân«j?@" õ›»Ñ?P°¤Ò:$r?¦‰TÔ3®?ØNX¤&ã3FGL J0120.4-2700@j²¸`™ËÀTáþ@_ŠÀ7âW5ŒªÀ:ÙP·¨xZ?î¯Xº@-•'ÎÏ0?þ E?z>`¿ÛôxÜÏh!¿àI€4ߛ¿Ú>«<7¿Ýï²!r7øAGNbll?¹¶º?°Vª«±ÂÝ?>Æimž0Ø?BgLÁ¯/ë?ÞG
–?°QýÖU¯)?î+£êÆb«?¸•ù;UÍ?oe´Êdò?û`Ù¾?«Ofó"r?·‹œŸŽÍ?ëïï|Ç÷[?©ã±¬³m?™e½‡V,k?Ž*·eëB?º'·êº?¦rnŸßJ|?ãÃô4EèÎ?º×àƒû†?'¶9­~!Ò?"ƒ}WŒþÏ?×âeÊ=U?º¯uKA÷3FGL J0121.7+5154@_ìÀ§¨À%_tÿ†]}À:›=އàÀ;—f=Kºé¿êz¸•)¿¹@
7¢wŽ¬×?ÿ¾Øà×EÍ¿éîÃà—´¿ÐåI=ê#þ¿Ò‡­rOº¿èƬªËúAGNbcu?î·Sg~ÒÄ?­N³¼uöU?oߒLO)?tÌ¿µËkì?¢ŒÐg.Å?¬(¸ÜŠ?î˜]hñö?²¶ì‹·¦?Ê¶Fóõ?Œÿtو×Ú?©ß{ß#º?°7Ykév[?î$œRå!?™rl_ë?'C‡õƒ†Ç?"<Õj,¢'?¤œÒ@ê›?"G™Ñqýj?îp‰Ð®ªO?)=$Í(V?]!âN€ñ?a²¨YX?¨Sâ¡Z¢?œÙx1²§3FGL J0122.8+3423@`Hüàü.ºÀ<€ÌC:À9ò¯ñʳÀ;x¢?Zˆã¿ð–G²œ@
]Œ©ÇG?÷Áˆ`Œ1Ò¿ä"ÉÑ¿áÔ÷p0áí?°DS½¨}É?²žçóUAGNbll?íèc.Æjƒ?³5KtT@?:×Rñ&_?AA»ÜsU'?°¢6ۅŽ?³2gS¾‹?ïÇ^Ý,ûm?yDl¤.
V?KÊÝ2!ï?Q¿ó"NZ?x×OÜ—?wg–é:Z?îP´ú3Dˆ?–4½6ÄgŸ?ô­`Ñ¢`?†™?¯Ëô?¢÷…—Nô?'@>ùe‰´?ï©¿<Ç?€Æ`HiX>ÑwŽT~'\>èA‹8%"?…Ž
‡&>r?€ÅðÅݝ;3FGL J0123.7-2312@gMó`Iì³ÀTmŽõƒ¥À9¤†ü#»À;ž_7ûÿ?͈–'ôø¡@'@'m€?ÿÐ1€Ö(¿êIÒ¿U¿É|ö«mŽ¿á©}~ÛÓ¿à+aé©ýAGNbll?ïÙI¶S?€PXýå?FwÁBr?FJߒ"4'?pŒy€î5:?~ú¡ÁÀÖÈ?ï…¼Z]À?¨Ì©êÀ>û?aÔEh7Þ?fL4¶'&?œô¿Ç°á?¨hT5û@?î½é#/îO?"Ä{½ÍIÇ?†Eti;]?sh¦ÍU &? !RM˜I?'kÒ¿{Ê?íÁª'"4Þ?	Ræ7°'?p$÷=È?pöÈ}	éÎ?°ðÉ#êˆ?œ½m`jÉ93FGL J0125.2-0627@b6"_õIÀPô'@.Ä9À:6¼ÿÐ/XÀ;×ÓãAƒX?ñGFÐôÏ @SU=õ"@©Ë€qt?ïj6&<D¿åĬ…%Ë¿æÇùG^'¿çƒ¬þPRAGNbll?ïh-æWoe?'ÝaÔdµ?":¡ØÊËe?…®å¦ïÁ?¹ä'Y[?‡pWm¤?îôšg¿¶[?¡¦	Š«{0?}Çd`Ä|?"uÃÊ?¨?™úÚñq?œ‡€pÛ?ëZïÝÓ©_?«pb±'ªI?µ)	wånT?£Ž4Eïl?¯þï2úb?œÂHG—Ä?éeÖz–?»~èz'¹B?­èþÔ¼ý[?¥ôFó"?€(ðè¦Q?·ð3FGL J0125.4-2548@i ½ ßÞøÀT''?àÀ À:Œn7ìÀ;ãKÊíñ?ä)ˆ[òð@pÀþãJh@	läÛ¿æÉ "ì¿Ö±yJÕÍc¿ãPÎúyƒ¿çBӃdçAGNbll?﹉ö?±n/Þ4«?:öí 'Ts?L'ÍÏýà?€áÇð·ïë?±m°M•¹i?îúÉâ*ʨ?¨€9ìj¯'?bQ¨ø–©9?k6aɟ?ž\Ž›"ÕÞ?§÷_›€y?îþòª?'§»ê~?"vü¼ÑíÔ?}‰Å?ijý?–ƒOösÖ?ŽekzæÕ?îÛ#‰›£ª?'U$"–‡±?q1O4*?k®¼Ú´°? 'à ?'e¦4/73FGL J0126.1-2227@g)Ÿ¡—ÀT6· ÝÞÀ9'r#3
ïÀ;§èÂ̙?æz–oÔµ`@Ĉ;Î7[@q'Iüο×:A؛Ì¿ä¹-ÔW8T¿ê˜mhÒì¿ä>»×S…ÛAGNfsrq?ïâÁl»ˆx?‰2ɒÿ«Å?V§ô£z"?fZ"`™¬ü?b;?J%Ëà?ˆ?-†Kká?ï"xÚi_"?'†3 ?PÏSôÉj?_ñÁžë?ˆÎ{)žr?˜¹c]Èq?î_]ð'eò?•1ö€ß'Y?"Ï»(T'C?ˆäÏ$_nú?ŸD†Å^¯Š?0=¯2ĝ?î›)$Ê ›?›¬0`Ð*r?h_k<²?fb—éAò?¤Ì§¼¤?›%KŠÜ(3FGL J0127.1-0818@b—ן#FVÀQWü€¿À9§¨Xy=ÙÀ;»ŽÐû«?ç¡J/¤‡@aé;îB¾@²ãàÈñ¿ãŸIÎD

¿áGk#|4¿æ÷Û\S
¿áNL•AGNbll?îylË×ÿE?«CEc?‡x?TÂÎ?Š+Nˆ"º~?¢‹#mOŠ;?¨é¼—d¹"?îÅ^ÌzÖ?¨!³¼Ë•?DüN~D?¶­>?Ÿç]®?£c^ºõ
P?íÁM‹‹,?Ÿ#v€»•]?šv$D¦9?‹p$˜Ðî%?¦°%F
?–S)ži?ë7ñ̖;›?ªpöÀz¢'?›ŸùˆÞ?–'ðŒWwb?¿I€ð?©Uz^Ð353FGL J0127.2+0325@aƒ&€IRÀM ªKÀ9LntQátÀ;hŒ'sZk?Þ8
(Lû@9rƒ«Ë?þce€À?ײÃ%	À¿àPxµÀ¹¿Ó҂4^g¦¿âÔWC~†AGNbcu?ïÃȱPuß?‰_†|ùÇc?SԘ›Œš?X"*%'/?y&Rž.1?ˆ-pàö-?ïW''\?"ü	ÑÆ?jjWšŒ_À?pœ
—-#?'ÑâçÍȈ?'Ã^|;?î‡à4¨ëw?'0ø1k?'Dž™cå^?'{þ¨n?¿ZÑ~«¡?‡F¾°?é‡,'VÞ;?¬±wðûWa?'bŒ&!Ÿ‹?¥ÏuÆóè?Ƚ$øBm?¬Mc¸[µ3FGL J0127.9+2551@`£ýq?ÀB%'Éä»À9¥Z'"ÃÀ;§YE³Æ?Û
ZÆõó7@­wt«¤@Ìc¿˜ñ¿çÃ&$Ö4¿ë涴BÎm¿ïÿì0€É¿à_ËÌ5'÷AGNfsrq?ïåù 
¼Ó?vÄkïñï¼?O"¦²ÁE?RrÛF¶»y?b&—H–}e?uuÃÓI?î½K_qÑ&?°ü?ß²ž?…GHç+?¡7Ü×ò²¾?³íRE¾?¥‰øµÐ6?î Aî0?–³Úô@T€?'hØ~ZÅ?ƒîÝIák?¤òÉÏ¡ïƒ?'2¾?ë¿«zÇM?´zÅX¥?ž‹B¡‹_?Ÿ
Ì
åE?º_Ó¢0°?³çÚt•=3FGL J0128.4+6257@_È
€CR?ÙØÀ1D,À8õeQ"qÀ;:-"wú?ì†ëÚ.4F@¯çcÑâ@	/ÿw¿àgÉ<õT¿åÕ=Ÿæ@¿å†ëabpŽ¿ïÿ‰OTHERspp?Õ&`TRa§?Åj&¢0x´?Ó¸1Òå;?Ä Ž^	èn?××çyÚ¹?Æ­XŦ†À?GÏró‹?cL.C¶ Ü?Ôß?
§ÀF?ÇVÁ?劜†Ïbú?Ç]­ñ˜2>?ޘAüÚôÓ?´¤•—Ëœí?ДK$?°r.ê¬?Ð¥)÷Ù{
?¯»ÄÞ¢'¤?ÇwñAžŠH?¥7µ—ò
?ÞËïWëñº?¸cKŸ¯´?ÕxDÉ"?´Ôs
?3FGL J0128.5+4430@`;ªÁ	J,À1݆ÀytÀ9ØÊUú˜À;Âٗ¶j‹?Ʀ/UÔ¦@ø|ôGe@¨À^Tt¿ã9\ZÒg¿ç™ë 02¿áۘ=_BA¿ë–ÞûðÉ#AGNfsrq?ïÇ6
€L?',ëAHЗ?YLÚWX|7?Í왐—?vÄ*!;#?xÊË
3'Á?ï†þ®¡¿?Ž¥~©Šú?eªÊ"Í6n?eώ,-
D?ˆÕ¡·dB¤?ŒZŒ'çÏ?îïÒˤZä?Œµ6µ'ƒ¤?Š6G?|…Q믋?•‹‡Q'?ƒkìàÇêð?ï1èÍÖp?ŠÊæ¤f¡@?\î›?V½[Ïb%Ú?—ô/??‰É­ [&3FGL J0130.8+1441@a Ç`|ÀGšÿË&ÚÀ:5O•GûÀ;Â+,Ôta?éÈŒZÒñ@ˆaq´ù@4NŸö*¿àÁÄ¥®GH¿ë¿ì¡ÿC¿ïb…¤ÖIß?êal×n¼AGNfsrq?ïÚAì
ú?v4Úû‹'?PökIΨ?Sã̙oFt?mCºo
²ê?tVqòðu?béo?Ÿ«eW³¼?`ޞ3µ?€–¬åôE?‡Àoç8À?˜Bž:èL?ìàÝä®&ƒ?¡Þ?Ü*d?¢
ãØ~]?"M‡ªÝø?¯ç>©Ea?™‡ù`J=?ïBiæ
ŠÓ?3öš`Í?T¥R¸`'ê?tsŸºX¿{?–hnȝˆ?œY]ikEž3FGL J0131.2+6120@_ëğס<¿òµQ€¦-§À8w3¼ÅîŒÀ;§' Ö9¿ëëQÑ?3ƒ@êÍ–*y?ýÊ€¥+ô¿àÈSõlö¿â~zm?¯ª¿Ùq¾óŠ°¿Ìsì.›AGNbll?ï°@NýC?‡b
ð?17žïV2'?2áßÚ#Î?ƒs2ôÅý_?†Ó"
A2?Ô÷8íż?ÔÍ'ù"Ä?'Å'i…? ŠXqO"?äîjMÐù?Ôµ^™Ò)?ì4þ9Øì?¨Õ/ö]n?' :Þdþ?…ŸFP¨ç?¹¯ÿy¦!?¥´çx9N?ï`æu.?ƒ©'<78–>ÿDµpÿ
?û©% T?"ô'ÕO?ƒ¡6û_«Ù3FGL J0131.3+5548@`οìºÀƒ<ŸÃFÀ:=0l¯VÀ;šºZ•¿ñ7`Ú5k@kÏæ1Í­?þv3þµ'?¿ëΐŸ‡¿Ý€Òõþç¿á#qKòœÀ?¢ÔoÁAGNbcu?ïáå9ÀT?yÒÒ:åâ?5hãi&j?6˜\¼­Ç?kmáYçm?y¨[|-Ð<?ï\O987?¤ô ^êc‰?ga"Eµˆ?tpð~À?šˆRæPBY?£A-FrÛ?î°ÈÝ]Ù.?iG¿ö<?‹0_¸.?y Ç×
Ú?œ`ÌI"þ>?ˆ-	J°Û¿?ïÃãgX?vŸâxh>ö"ž<è?	µÌ+?}÷àÒkc?vž=¨Gfw3FGL J0132.5-0802@bûw µíÀQ%4ß۝JÀ:ˆÉûaÀ;¸A›«Â'?à :M·³@óˆzãK?üÚß_ ¢¿¶S"F@g?ïšÎãõ«¿ÚÎOT¦ö¿Ðà-ëSSBAGNbcu?ïäcÔ]Ý?i+qv"©?<.ô¬f°º?=ˆm­­K?hƒ–L!?gï×_»µ?ï^ؚT<?˜Õqu'(?lÏÿ-~ø?'Îà}NŸ‹?ˆtJP?Œ¯X‡Þr?îŸim"¡?b
`Ás?Ž®~Р=)?–ŠÙ¿É?œÆóiÿM]?‰Û­?ßE?í"Íš"½I?«ýAê-ž?ŸðrßxÕ? ‰Sn˜?¦»Tnò?¦L{
‹sœ3FGL J0132.6-1655@ed@ò8—ÀSÁýaÀ8]à_PÈoÀ;Œ­Ánʹ?ïj
®ÀÙ`@홟£ÉÉ@pê¿üÚ²¿âðƒÑk¥¿æH @ÎbŠ¿éQØXNÔ¿â—!B¬BAGNfsrq?ïöz؝ë?KUuq®¼É?8½ŒK@?5®4îS?IµÙسŽ?GqþƒÏ?ï¬ßIž‰?DÂ9ѧ?J…°ån?SOu¡?«?ƒ(=Oi"?™ûy·{?îå>¢—àÚ?²lì–Ò?†^%-ýñ'?~'ÿ±€w?˜)ëõ?†Y${Ë?ïmÕƝŠÛ?"1a›î¨%?H7vï£Ï?Q¿
:™?'ƒ‹tыˆ?"ºg'êu3FGL J0133.0-4413@qy[À6ãÀQ½²_Μ±À:/ĦãÀ;üË+­-¿äP/5€H@@$³=°@?ü¿ÙŸC¿Þ jpX¤ÿ¿â~U<ê¹i¿àÈÇL/Xˆ¿äJ‡áò_AGNbll?ïВ"ö?‹~ÜÔlË*?F²¦òb?e›1LG'N?tà¨÷Üf!?Š—dÔÁ¯á?Ƃz?'¤Ü>	?VM…F£"?`6ò'ÝÙ?ˆT¿î?'ÞtT';?îMò RI?"_uòà4S?Â=^Í7?$°И?£0Q냼8?'ŠÓœ	é¸?ï¼Ó՘á?"!F³p?C7Ú¨xq?C&3)nª?œî¦´g ?pLé"73FGL J0133.2-5159@rˆv\ÀOö¸¿ÏŽHÀ:pƒÇ ="À;î£~éпÔâHæ_R@õö`X@kŸ`X¿êu«Èg¯´¿ã8c‡'Ç¿íÁ5
—±ý?ØJÛ~SÌAGNbcu?ï󭭑Zp?W»(8|?L³MyqjI?KÜòoÜ3?D•üA$Ûû?P†Œmø›?ïÒÑ©ý(¯?yÈ:úËv]?C%'ƒ§?K"³¶Žœ?t#ˆ|»X?x(2•"?îq0rÀ]–?'¼
[O;?'‰S>–ý"?"C¡j5.p?ŸPži]OÄ?‰ºút\Î?ïÌÓ䈿?{#{‡øî?#ùcóºî¤?>!<HÁ?xö«îÈó?zô'ióÍ+3FGL J0133.3+4324@`^œŸr÷nÀ2Ш߇ºtÀ:BЏ±¹À;Ԓr]ën?ÞÁ4]·ñ@¯ùO·£@h~€
¬f¿Í´›â&Ú¿éM$ÓknÛ¿áËÈ­zÄd¿æ9'%y-¶AGNbcu?ïÂiSkc€?Å^2º¹?W:aô¡¹?X+1@L;?xüÓqÑû?~$†£ÉÆ?ï2µA,`?š¼u!ʶÖ?uô•ìȹ?wiÅ¿Þ¯?",2žAá?—xz@¼?îT¦D]Û?"AòÑyX®?"‹L³²?…IШ[bû?¡(Uóˆ8w?Šœá?î	- âüì?žâH&:ù?{ÒûÉyB?u†@ä$`•?¬
s'W ?œŒ•j Ø3FGL J0134.3-3842@p¾àP7PÀR×"Àh¡À:E©¸ËŽÀ<jüY'¿è"íŒò@tM¿%šC@¦H «L¿æâ.ÝdÖ¿æÚešA=¿Ð·½å4¿ëøÎEGݺAGNfsrq?ïé6·?kTj0ŽŠ?Oñ#}N7?_£˜W½U×?^ny=íH?dž;K"?ï¥s[ž?†µŸ
ªj!?QÞ4åÞÓ?VÔ§P?"'u†m>?…Yêz‡ù?îºäZ0²?'›üÕ=̉?'|R}¶G
?…Ì·»Üw?—'"A㢮?ˆ5m'žž?ï|&®Ò€>?‡{c=»Ðc?+2ÈFœÍ?5`0#yðä?Dĕ"Ù	?‡Nöú—˜3FGL J0134.5+2638@`׃¡	ÐcÀAŸT_Ó¥.À9bÒX'ƒÀ;{"qê('?ñÄmO¹¦ª@>¿Ä¦Ž?ÿÛg_4Ã×?ÑEÉïˆõ™¿Ù؀	O´ô¿ÝTžg½1¿æí¤èFÏAGNbcu?ìöRÄ/³?³{®T'W?§l^'˜¡?£ Ì¿4'?¯.u*l)?­÷Õf³?지òO©?±
Z]nÊ? Q¢ÌcŸ? /Fށ%Z?²›wïPë?ª q¼-?êe…Z&'ø?¯Tå: CÏ?¹iq×úö;?¦¬×'‡"C?³jcVÓÊ?ž²±ºE¼?æà˜ÓÐü?±Õߊ•¶Ý?·Wº^?¦Š›{—?ÈÑ¿°`Ä?±PncҁF3FGL J0135.0+6927@_°ÄŸ×¡<@¬Æÿ®K'À9ºGº©´šÀ;O‹Ëz½?½I¢z,°§@Ó.ö¸ƒ•@tcßÎ\D¿ÊIÅëKô¿ëÂsÊý꧿å¾ësè¿äU÷i"ªAGNbcu?ë!¸‰µ?ÀõTÃ`j?–üøËD?•²a¡íϧ?À¶^:('j?À?ë
bzz?èP"rF×?ÈD³}}ì?§²
4;ù?¢³ÎD?ÊÇlð]$?ÆJù-‹IÄ?êªÃr¿k?®œÚgáÎu?©Tò«|+'?"û´ó‡þ?Á,GU÷m?«9@
óyy?çñ0+oû¸?°âá¿é?—f–ø>?VޚÆ
?ÍK]em2?°È²ÈþÀ»3FGL J0136.5+3905@`9à`þHÀ6ñ§Ši{À7p͔ré,À:sˆ¬Œ%?çKÀÌþÓ@‡&°:?û!/à˜[¬¿á:p'2¿×ᾨ·¿ÒËjµ^#Õ¿Êþô^®ƒƒAGNbll?î;Æ0&?©â''»S?lã6´F¯?rHûcÔ«	?ª%"1¹B?© ÚÐüÚ°?ïOTš¶.? M­¸Òä£?r.Dpi‰ü?~¸œ‹ÖX?'‰ÛÝ?šðön•?á)MµÉ7ƒ?¸¦QϞ¶I?®Ý¬™²Œ?œ<`v,ǜ?ÙѲžÚZ¨?·ù*Ë?IF?âÔß夶'?ÀlÔ^3ì?yý4æVøº?ˆÎ€ë-s?ÙîKa6ú?Àv+EÇ3FGL J0137.0+4752@`Yi ­ŠÀ,˜¥ÀïHùÀ7²MryšÀ;ªÆè‡=?ú"ç÷²@WK@î>¿àä-R.Ý¿ä¢jT¡[Ê¿ãùÁˆ(¶‹¿èãÅYÇ¿AGNfsrq?ïÙ®ÁË_i?fÌöàP£?Vˆ€ˆc»?SGé˜Ì?kýð'æp?c…¥ßþ»ë?ïÁ}¸?N?€h†Ã'Ç?QîˆQR­€?U&ºsß?zø‹­"?~#c€tò=?îDgcw?š?`¾@œä?›ßh§­¨?'¯ÇH[-?› Jl‡Ã¨?'@RØÌk\?ïÖ°‰qÐê?zÖ˸«"?#p¶ªU?8Ξ&ûÕå?t5–Ú9Õ?z¯Û¶ý…3FGL J0137.6-2430@i,ÀÒÇÀSÑÒtwÀ8柱mÀ;ÀØi¹>?ﯟ%°ÏÒ@ŠVf/]@$ Tä¿ã@ÎØk~¿çCAj¦¿éi¶¼Xû¿ç¾ãèÈ*ýAGNfsrq?ïô›[]?^RÃë¡ ?BW,Í%×U?TAe'×´?MŽeÆȵD?SEÑfœW?Å«Ô?•¹Q¹q([?Sàgà'?`Û2ĞVÇ?ŠÔk!´.å?"îøɃ'ê?îä$ÊËø?#ÀMVZ?"Ð\¨Ÿ@¥?umš]Qß?™8R1[£?‰2¦‡'0?ï&ˬ ¨À?™ÄÆ#0-?d:'š<ãÜ?e"7©-M?˜ŸEˆ£K_?™R1÷3FGL J0137.8+5813@` Ç1¾À\l.NÀ9Ý:ZMÀ;OZˆ%¿çê3!añÚ@Ü¡jHs6@u8_—ë¿Ú¶½Œ'¿äå?æ'šV¿ÞÁ¤G¿ÜO³7‹˜¶AGNbcu?îw‹í)?¨Çt¿.?wšF!!!?s/®é¶Ù?¥¤­ä«R?§@
>›ò6?ìÁ5feý?½éàš­b?‰@º…ʏ? >¸Q0æÏ?¶Î=|<×?º³m-Rã<?ì'¨k'˜?¤-VâÏ?¡J€«÷&|?vÔÄ°H?¶Ö2f«0? §2_TØk?íö£	'Ï? êš»Ä.?Hpä
/ñ?IƒWÐ.¢?³Oi¢c}? Þª%åœN3FGL J0139.9+8735@^ß/@_k @8ÇÞàˇRÀ:[o¨.‡ÓÀ;Óác\ƪ?ÎcJ]'@
èO-°7?þBŽ_Ô¦á¿î¿?97z?Ûd˜nSù/¿ã"=êZۿŬ†6́	AGNbcu?ïã®QÛj¡?kÆZ‹zíï?Tš¨Ò:Û!?SXqՋ˜?bY»wñ?gŽðvÅÔ?淪͖‰þ?‡,DØû£$?sê›0D´?uº»+a?xIþvLç?€zÛ'×QD?ï+ö¢?ƒEšRf
Î?…|Š?ž±	?v/VÏDbŸ?Á88¸ÇÅ?xÑCyø?ïc4LÛQ?Šê_Kö]ø?€(v\?äK§SÕ?‡
ÞR¼æ–?"&—aòc'3FGL J0141.4-0929@c╁$ÝÀQ19Ü>ZÀ8~ê–pÀ;Rùþ?ÜágfÊ@\ÀÃÕ@ûª ¨»¿ØòvÅf/¿ä1Q÷zÜ¿áh'N4§Ž¿ãÑi—H[ŽAGNbll?ïèùn¹êå?udçü݇?&FKÞÅ/?$gÜez$¼?e¢,ˆ(Çû?u7çí_¢î?\›<ã?ˆmý¨åñÄ?UGaÎA£j?\@Kôð?…j<Ÿh"?†Äɨ·è?î—ìV‹ –?"\…Ý(?‡8üˆú}ä?}ɝ' ò? ²ûuW+?1'9"[?íIWG"?¥¼¿5ˆ‡?cøx·/,Å?c Z;(?¶ñ€
©ô?¥‹Ù¯y3FGL J0143.7-5845@r'@$³>ÀLŠ+¿¡kÀ9)–‡å<À;h¦©L•¿úÊ+lë:Ì@ƒ§>ó±?ýj*þÜ>…¿Ù²ðm:ëä¿Ú`%¸)¿âðZ›ü¿¥Fÿæ!)AGNbll?ïùÆ!4?BŠÅ;Ö£?î€F?EÙ«Í/?H¦Ê
â¹?AžÛI·?ïÔÊ·]à[?uBb?½4³?BÒ¦t`¹?Lwg#?s@O'ƒ»?sXoûzý?îÚ•£ñ?ÏíQ
ü_?Œ=ÙívëP?ƒÈ"è´ŒÃ?–ˆÀfP?ˆ7]ÈûÀ?ïÈd(3¼?uÒ<,¢…>Òï¤Ng"Ì>ætsq{)?{É/ýh‡ñ?uÑá4˽Æ3FGL J0144.6+2705@a)  ôØÀA%ë`5ʽÀ7ÙcaÏ'ñÀ;a$WÎ?ò†¨ÀþãJ@D8"*@kïð=jD¿àK\øÜþ§¿ã_Š±
Bx¿âÕAVÛ¿ä —YAîAGNbll?ïÒÿéí8?sèé—áÔÑ?/¼ãôLNu?1Ò­Cáž?u'#éÔï?s¦Hí±Ïo?ïŠ|¶ôЃ?ˆ|º¥Òø?]ð…ІÅ?`$2ÊY«?‰À42Îq?†»ïß­—?îf¦øU%U?˜>+f¹ ?ŒÖšoêãE?ƒ' Ç3­ö?¢_éÞ²ñÜ?"p'Qˆ?í;
¦?¦°ëö§\2?tè칕Ð?vërT¦?´æ¹	/6?¦vÁ²*Ó¶3FGL J0145.1-2732@k>àŸèh4ÀS"2_Μ±À8ŒpUÓq,À;«ô5Çb*?ñâçæٓZ@ýˆšBáÒ@Ž'`:'n¿äs'¹áÁ.¿çódÑfs¿èîÉëਿì(LQ"™AGNfsrq?ïÞ°|¸©?y-D]:õw?Z‡Eº'?[B®MFPß?dGº÷¤yy?w…ñ1#Š?ïŒ"ʺÏ?–Í|þàþ?Oòö:w³?YÛ€c?‹øí¤Ï?–.­ì?î½é¸ibS?'^ogmú"?•ŒkŠ6*¤?‰€(ìò^?'¶]h‹?"Ë9Úס?ï"Íl­?hŽ9%?S1¾º´›³?Vؘžb?Œ""çNA?â`OÉ3FGL J0145.6+8600@^üá~4¹E@7<ö í¦À:@yꧩ'À;Ú|öË£Ø?ÍÏ·úKO@e™
©@&«?ß>¿åL{7-ê¿á¨å¨P¿æØþ"¿æ¦_&oðAGNbcu?ïcœñèŽQ?"±í;<cS?'nɗð ;?†Kr61?"©ùíìKv?¼t‰oó?íýb– ƒ¨?®0êò]Ý®?£ø;eàðn?¤ÄۂžñÅ?˜c6`-ª
?Ÿ`§ë å?íÛoèÚ)è?š‡šþ©§?™++hÝ?‰^7ü±In?¥ÄëÜ©Xø?"ù[ =oL?êā–´þ»?©æ±‰å†ç?¶%S'Ê÷¶?¤ku­:~?³¶ŸÇt?¡ð2‰M#¹3FGL J0146.4-6746@rqú?̞ªÀHB=ÀTïFÀ:4Ò{bvîÀ;÷õy"@"¿èzjÉfT¸@
ÂPŸªª¹@ )`vP¿ãµ¡Øà׿åFGž¿é=uó»è¾¿Öb¤æåãÛAGNbcu?ï}¤¤4š?'‡"°/¢Ž?erŽmÑïH?g,՛ié?‹_s;~]O?'S$a*'¶?6?€û?†óÆìrËi?TOŒJÚ
I?`€i:ø—?…QÀæÄÍ?"9BsŒü?í½Œ7åR~?™åÔð…f?"|§™î?e?'®å9²÷?©èè´³¸b?"À!íý?ïSh28ÁJ?Ï?ò6??Ùÿ|ÏÒ?H§ö£`Ÿ"?•'¼}ã¦?ÈÀï,3FGL J0147.0-5204@q¿?á—_ÀOz-K6À:=ƒJ¢»À;þ0íÖ¿íÊ֗?»ñ@:9/K@˜¼ R;¿Ä¢¾lô¿âð³¡á¿ç†kEÿÀ8
{Œ›ãAGNbcu?ïä;—ØÅ?l{êÑâƒ?SßÓÍÖ?W™ûJ°;'?aÕâ!Sø?erØCm?ïÑh
'?wÕ\/;èÝ?C÷¡ƒòIá?L¢A;ãÅÝ?tÍC¸«™?vI8Ÿ@¾?îa6ìAˆá?"r"Èdh!?—Ë"Æ(g?‹›œÃ,Z?œ
ÿ±¦Ð‰?"ûÊ«Š8Ü?ïµ»ÊtŒd?ü~ª¦?ìñô‡9Ü?$=[ó?'i3~óØ??âï|P>œ3FGL J0148.3+5200@`xwß (À#Ä9 1xÀ9¸þ›{ñéÀ;%îÇÉ?փՁò"@cFçp?üRóÀ+©§?ïýìH#k{¿¿Î'¢À¿ã¢+e"]g?¥©yámmÂAGNbcu?ïâÝW8× ?jõ(A*?PyGMÑÓü?Q
'Œ_Ü?dæ ?vo?f'¾+?îbˆ#1
)?³ô¯Ò«Ü6?vÁUU˜?ˆ€*t[³?¦ÿS"M¬¥?±™Î9W?îC"ÝØ?•PMçÅ}?–‰k|Å ?‰¿û¥? ‰¡ió¿ö?ŽnÖ4ðØ?ï:'·òÝ?•ìRm£hk?WàæÈèB?añéèî ?—=\s ?•ˆÿhïEc3FGL J0148.6+0128@bÝ"ß°Õ ÀM †¿¢AßÀ9ÀX·Q:…À;ŸŽ'å".¿ÙXim×ÉÖ@†öA»6L@*@\fˆ¿Ú³ßæ…·¿æ—Oß³§¿Üvpd_¯¿Â•Òÿ[AGNbll?ïöaœ'ô?TW‹ÔÆ̕?z½$^à?Pð: Ù©?QeçÝÓ
?SV¯ˆu×?ïÑx:NÉ?xÅ›ø'1?Cþ'÷/?NF=«èõ?tÄ æ™¹®?v˜"Irͪ?ïYê†ÂÍ?€ˆ–Øu¬]?uÉO"vÔ?fþ4%·`s?Ž Õ§½á?z­±¨Ÿ
?ï›NëW´?€9Zýç?fF	\(?í³Û[VI?‰CÒ$	Ú?€î9¯© 3FGL J0150.5-5447@qÚ®_ú;›ÀN(}?Æ¿mÀ:ÎakTâ°À<*'ë"z¿þøYÐÖÇ¢@CpcÀCÒ@ò -1'¿íïÔ.ž"¿Ý¥Zõfkf?aBàÖl«¿è2£Ý¯AGNbcu?ïÎ'2|~?‰N¥?pwɉlD?…ÜËFØÚ?`ê©ðo¬?hÔ¿ˆó¬?ïÎ	‹¦Ï?z"iyÿ?Fvš`?Péu™F?v,fì5])?xÙ·Fmž?î»ÝÐ7Ø?œØ`§b°?¡pxã%??™Î˾ÐÇ=?›£T2ºe?‰b"ÈÜ¡Í?ï۰ƏŒZ?qí2œ<È>æWƒÊ둛?	f`	/Õ?rpöT]"?qèH#j3FGL J0151.0-3609@oƒÿŸ‡ð$ÀR†À
¡©À:mtòd/À<gpQ¡³Àæl¿@+-']¶@¬]·ñ¿çųT
{¿å5m:ž•
¿åžçsŽr¿Ö"½.t1«AGNbcu?ïéŸ[.s?oR+'»?GíS¥\?g¬æØ?a7e_<£ß?b\7æ¼Rº?ïÆÁ׉ÆÖ?|±Ë×ú+?DlÃs¸«?P)
þÝ-"?z{Ì¥'Ò?}sÎQ™* ?îݐ²(œ?"žg¡yÂ?'©Ķ.?}®(¨ú¯?¥¶Ò4û*?ÆŒøL‡å?ïÖ\ûã²?sۄX€Á>Ì~ƒ¦
G>ãÒ<<¨?tÍò>e|?sÚN¨àܛ3FGL J0151.0+0537@bœ] l‡ÀKK¹ëÀ:o¢äßÀ;Ӓºǿޔ®tl}@
w¼'&á@@ߜÿªšž¿ë<TÞÕ¿âA¾¦:ß¿ßlsñTl¿à÷ŒŽ™5qAGNbcu?ï°"9Ä/?ŽéG3ÞÙ?EÚåjv?Eùa2Yîÿ?'¡É ˜Si?ŽqÚe«±=?ï§yäÜ?†©éd(ò?XB¨"Yww?hy"iF{j?ƒ7$û™Ü?'"8¾ß"?î+¯nŠ^×?•oôSáÍy?¿	±@º|?~Ëù{";²?¤å">¹µM?'´TÁ[ê?ïu‹÷?Ú?‹˜ŽN?BýÂ0Í?BÊÁT«ƒ?ž`n"[)?Šß
I.3FGL J0151.6+2205@aœ~`Ï6ÀCU˟¦#À9½#nšÀ;º£ø'Ä?áÄDã‰Ò§@š§_Tú-@;[áF׿æÝÓG7p¿çݶÂs¿æœÛàæà¿ïÿ}¿|AGNfsrq?O.ä?ÿH㡤?uTæÿ'Yt?w÷ï€N4?…&ˆ,kÆ?‹è]*Z&Í?èÐtz%Òl?¾ãʶúz¾?³­&ZÙ?°<-í^kª?Âç›;«à?¸I'Š}2¿?í­¡P_Â×?šõú#ùðP?¡ÁHt#ˆ‡?´"b?£d¢…àJ?¤zê<!
?æåq—?´{ðÛÇB?ÀRTÂ~"7?ª‹B'GR?Åqc§»Á?°œ\Z 3FGL J0152.2+3707@a
¢À8+À~à±À:>'d@ò9À;ârÚ/­¿Â©—âùùš@&¶£Ã@@vÀP½ˆ¿Þr²™3±ø¿ä®K×¼6t¿åˆMD+~¿å–IÕ$ùÎAGNbcu?ïzo%z
?Ž€pè¢jâ?{JZ}š?€ÕVLPRê?ƒ¿©ô>?‡d›‡Yþ?ïK
°Og?—2õ<wèÍ?sBs»•MÔ?zË0—Qq?'Î!û¿Â?'Úè•ØGå?íüÎ:lX­?—1¾còQ?—¬˜Œ«Ì?ˆ:JºŠŠ?¤\ÐúŸ<?ü˹±ã?î"Ý YÞ?"y
šž'd?r¦:r›ë?g{zÇð¢?¤]f¾ìº?'²QÚ÷t3FGL J0152.6+0148@co€UûµÀLÃ)ßÍZ'À9qè
šó6À;rÔ#&v?'¤ŠŠô?v@'˜ª†Pç?þ/žÉ.]¿ã}ûüþ¿ÎU²;Hwà¿æ1ð\7Ó¿—TŒQæ_AGNbll?ïn[¾u5?g]¯
-?gÕßÕ}K?iu ¾Ö™?Žs˜¶mSÆ?Ž0ØLc?ïLJ¹õv?zoÑ|Q[?G–‡©e\A?Nbƒœ"YX?yIR†X™˜?x}_ä"+?îÖKÔgp?˜N@oHhæ?˜¨y;߀?‹_ìÄMÈ?¡þ™†™2?Žžš3Ó;W?îÒ³îÿEÚ?–#~ñJK?Lô-Y$w
?Y²´"²ßä?¢`ðZ§š?–$Òrœ4+3FGL J0152.8+7517@_¸Ôýó¶F@)ÈÒÀ+ԚÀ:–›¸WËÀ;±"Pª<?ï¤ãŠå‡ë@1­@˜?üS ?ïD¹®j"§?£«ÁlúÞ¿Òò-¬-}¿ÛZâÃÈÛëAGNbll?ï¾·¼‰[(?ÊÔ¥ú_Ä?iíùR¾ð?}½K¨ÂÖ¥?s­%NB?'¬ª³(=Á?íiÄSKeÒ?ºuç'{¾S?–ùrÆli?£ŠjBå(?­ç:'ælÉ?¶ÀTù@IÀ?íü€«Ç? E¹‰? ¡m•o÷l?'-Ò:ε?¥~Ê_ß<-?–Ž»ŸÌ?íU9&þ@¬?©õ`´'?¡$&3ú)Ï? ¤ñÍÚ0?©ˆG\!Ëh?¡££íV3FGL J0153.4+7114@_ûÞ¨—c@!òU¿û?À:Fó½Ò^À;¢nfåè'À›	º"å%@ÎkéG'?ù~àZÉ$?ÙhS.-î¿åVüæ¿Í$Àdð¬¿Ð¡}ÇñØAGNbcu?ï³òé~þM?"^&Þ_½?5ª"¯ÀÚ­?3hÑùÔjM?'UðúÂeý?"0ЏŽrw?îIB-cIÞ?·£C‰j­?jâ2fŸ¬?t¾'&ÏÈ?©½ºapƒ?· !Úõ"¦?î.aã».‡?˜×ž@fO-?ŒEÀ2F?€oËÕªÞ?¦›"@†!?•¶•GÈ£?ﯓV†â?+r€qr>Øï×W²XÝ>è¶åł%å?"cŽÑL?~ÿðÙBé)3FGL J0154.0+0824@b‡…À3aVÀI® ö½À8)+rt'À;
ú滋\?ò…­¶Üöf@¯í|Å£c?ýÀ(~ú1	¿Ç'ދ'A¿ÞF²ZÊ¿Ó=ЊòaÝ¿á>qðˆ=ÒAGNbll?ïe.¿S??"Wí5ò
?g	7–P4l?iŠ•Ë&X?y"Î
?'ŸN[e¡?î¯ò½@"?£;Ññ"€?'xæäv¹'?Š6뜎J? bšrÚu?èÂþÖÁµ?ìh¾V¢`'?¤7â¡6‡?¢ysaëH?"ö–äã¡h?³}}'<Ð?ž§jsXŒ?å|¬•ßx?¶39EuÆ?™¯â?˜·òtbë]?Ô_›¨´Î?¶}¤M
—&3FGL J0154.9+4433@`Õø@À0Ý¿Sg†À:_`¸§|À;ÒËÖ,Çß¿÷1ϨÊ9@f.fš¾³@w€ KÏâ¿ÞzùWf¼¿âÕ
Ý}
¿è"õïʗ'¿¸b
CVÅAGNbll?ïðBq…ø?d¬$´¼•>?Cì#PÑ?OQ<H«?U…d=Æ)?]öC™'¶•?ïͬ§SÛ?{Üpìî{?OÊÿLHÙ?Y¼óƒkã?u0LMò?xmtÝĶŒ?îå¹\‰Ó7?ŒÈH.]?q…rýö?'ž	\mµq?"àŒ
?âzÚñAÕ?ïî#¶âÀæ?a#½12Ð:>Û½k±·Çi>èÖ~cY|?aÎjgf>?agû^MÜ3FGL J0156.3+3913@a
Ô2TçÀ5î¬_nû`À9ƒL8½¶¯À;Ë+/X³À¸ûh¾@(³Ä"t@öA?»VÙ¿åŠXµ	ð¿è_Pé/6­¿à¯öäV	¿ïÿë‹åãAGNbcu?ïԑ
ß2?¨÷£×4^?*Å©ö=¶[?8LAÁR–?táMh^y˜?¨öt$Î\?ïÉɪeG?y*á%ß?PžX,þ:?UÁ$Þrà?vé»\B?v:úzGâ¼?îë¢!ó
?í¯?‰Zñ¾¦M?yÁ
zú¹Ê?•ÞDnœ?‹©ÈEÍâ?ïðù"#4?e‰š\ò¾ø>ç…]ÌöÝS?|F¾™?]ÝÏ©&?eQáÔGþ3FGL J0156.9-4742@q6`ÀiçûÀPp×?íUÙÀ:õ©ŽÚ"÷À<&¬k-v¿ö¹Ô,g'@†Q
^¨­@¥ßx "?ü­–‰¿ïiŒFR}Y?ä(_ÂÞ6'¿¢·JüÊã¶AGNbcu?ïåÝùZ(ç?ƒpÈ?Éÿ?9Þå	øÂü?O.­ì§ó?fæ*˜ä?]©…KÁy?ï؄Œ)ʧ?vÚCжL?>ÍoñžAä?Ia#ª·ú?qÐâìȸ?t_8N+•,?î 9Àƒ?›&à˜â"þ?'SšW?‹ô%ŒÑïÒ?¥o=1óL?—<u¶ny?ïããÝêÊ?q'ÙXRP>¦•ÔÈ$m>Ç￯ë]?l¸·èþw?qùÀÙÍ3FGL J0157.0-5301@q¢ß?–ÀN°ŸõÔ-À9ž´À;(Âz?ò¦Ì,¾Ïß@Œ,ºÉ1?ý*
h¦?ÛM{'ƒ·¿¾x9cN¿Ì5¹åg¿æ WÊ}AGNbll?ïqktõÔ^?&M¬!¡à?}Ä817"£?~Ⱇ•"¨?"éïë?…ñþA*Ê?î÷,@z–?Ÿ8ûÍìOó?{»üѕõ½?€7Ïþ*L?š+x¼GÂ}?›ImÂÍ ?ëÅæn6;E?ªÆÐ?±§­Ê$? »l/FÎÓ?°)ÀŠ [¯?ŸÍç»Àç"?ëÅÁ`n3?°C»n°»/?šKi»+#?–oŽ+œ?»?Ä]­?­€¿ŠO¡N3FGL J0157.9-4615@q
?ÐÐhÀP²uÀjÀ9Áj©ÂÉÀ;çl¸ÿ?ðÎeä¶@H'"Í.Ç@˜[À6ã¿ÞôË·"ž¿çœû7昝¿æèf">®¿ïÿëÆj»"AGNfsrq?ï	àgÇÓÐ?¦°i½NH¸?‰ßàÏèÎ?›å†Tôƒ?'Ô'š?Ÿ_óp>òÛ?ë:(AÀŸ?½DõO¸Ý?¨ø8'éc—?¬Rü‹á ?¶št}I1?´fW£gd?ì_€ÆJ5Ö?§³LVL²‡?°´"îþ? n¯ˆ2u?¨žË½`fv?—èÔ´†"å?éƒé"7í?´xµU‡@?·'Šºâb8?¤àIìI™Y?¼Àø{Þe?¯Ô%ÍWF3FGL J0158.6-3931@p,Î?þó'ÀQÔÀ_×,À9XŠÙã5ÅÀ;Ã¯Ù`?ÞÖæü£Õ@ë«/™Ì@.HÿxE·?q×U¼Ê÷
¿ávþOž¿âÅ
¬N¿Ù»+ÅUµAGNbll?ïò2ïv9?__î*Çùý?0^¼pRi°?(5è\¤?W'q÷¼ô8?^Í·"²«?﹖l'€?€æ'çÓ-æ?L±Z:p/(?Tßú| %ê?ž†ž9ö?f>9?îÿÃ7©&ò?‰éá¦"
?ˆ="ãÉž?}lmOWN?"èÏö¡S?ÿ>µHV¡?íø/‹Üõæ?üÔÔi?`w˜ßk̕?d‰˜zUÅ?¯u´9äÏ?t —ð@3FGL J0159.4+1046@b–¯ÀL‹ÊÀHT(?º*3À9MPíX]À;€¯°î¿Ð	'û%áÍ@Ê#EÕLM@èHÞ½¿æ=ô$™V¿á©'¯èˆ¿åãtó·¿ÇÃ\ôÖ3ÜAGNbll?ïè_ñ˜"?e¶à[?>£#ZqC??0YN³÷?c˪‰$O™?c PíUcÉ?ï·ú+½S6?€ººt‡¢+?IÄy	²ù?QÈäÝÜ»?€e-wª—9?ófÇxU"?ï1JÆO[ö?†zùg@?'©³°¼½?x'Jhï?Í®¼"Ã?~Ÿù䕎™?ï>>'´?‹:Þr~ÆÜ?*Æ'¦d?4	>	VLú?˜¡·†/?‹*ËŸ"3FGL J0159.8-2741@k`–óEÀR´›€#¦ÎÀ9þ¹=£ÏÀ;ضXí ?î!J˜]7@Â5'ÿùJ@JIÀ4¿ÓdTªô'@¿Ó§¨Ì£˜\¿á-=…œŒ"¿é~"لý<AGNbll?ï^'º7‡G?´NXÀæ?‡Pk$J1´?'lh'±ù?
æMÓü\?–"ŒÉRs?îä$®&ã ?¤,ØçûÕZ?wW«Z¹¾?y s;M›§?¥vŒí¤?£'"ÈW×?ìp:q«ý?§ø袑±ß?±ƒ}e†–ÿ?¢Y4ö¬?¥õ^2ú?—q+™÷?íPT_Žî?¢b#
¢Â?•´Çgtô?‹z¬Ô½cû?°+)²«‡?Ÿ2˜Ãác3FGL J0200.9-6635@rGÆŸ¸ÀHñ7À:/œÔ·|ÙÀ;ñò¤ÍªB¿ï)÷é00@î#Ž¥u@¥ Z¨î¿ãµ¹óA‰¿äÔÂâ4µa¿ç+À"‡b¿Þ(>Ã4G°AGNbcu?ïôEŸ7?SLù3(?5?ä¦å?4¤†'ÿ"?R"{—׸ú?Q Ï"s7?ï¼xã»­Œ?{ÞØÙåh?G
Ñ>Aå¢?M
ìIÕí?~áÓú`ýz?zTêsõ"¯?ï1€[K_?ƒQß2+ïâ?~—ª"wM?lÛ*Å?'*	ñš–j?€<É2?ïÅ'Åî'?sÂP%:FS?´Ê3œ£ñ?Òÿ»îÁ?})JGºyž?s¬çg]"3FGL J0202.3+0851@bݍ`¦3ÀI/ÿ¢/À:€\GÿsÀ;ÕiŠÞô?ï+Í+þqÇ@
=`'@as\f³?ïÿ—›UÊ¿àZ¦íÈ£{¿à¯€`¸}¿éo~ýOæ6AGNfsrq?îÕW­!æè?´ƒö*Ñ,? \è´*'?³$o¿jñÛ?t¹B)k6ý?®`üqKð?ì(J0jnd?»ìtúšà?¥=›k?­Êöÿ¦™	?´àù«WN?±:"̀@?éÒw){æD?±§'°÷¨"?¼'öÉVs¨?«m3©W}ï?´ÙOêÊZ>?¡T»Du£?å÷´»¾¦[?»²ìÞþ;?ÀUuF F?²o«wº?ÇÌ ›¿FN?µÏz'$3FGL J0202.5+4206@aԀuÀ2Öÿ_ÇôÀ9臢 PØÀ;ӗù†i;Àת´*8@z*ßQ´©@4JŸá\Q¿æñO:þ¿æêPé|…ã¿Þ#q_Ïڅ¿åíTW°@AGNbll?ïÞý‹TÊÆ?o•z¿‹?:aT©«?;Ÿ€b<Ñ?m¶S@´EN?nR&8¹J?ïƀö:"î?{}ÃÿL=?Pú[å¨3Ó?TFþHXíö?x€íéK|?xá:OÖ¥Ü?ïWɽM±?ˆ1K¢ô»?}J6ùø4H?r<ºƒÑ?•¢y	Ø<Ñ?"î½31?ïæðÅjä|?jß
CŸ	>ÂIŸÅ[GL>ÝÑ`öÈÿ±?i
¨-*,«?jÜ/É[óº3FGL J0203.1-0227@drä¼®ÀMøK¹ëÀ:hØÿ
6»À;ðL'8¿ö+?(´Õ	@ُ'Î@€Ÿ¨Qm¿ãÝêŸÛÜ¿ãÂ73&¿ãJ<ɦ¿íǔdâ"AGNbcu?í\wCþÎB?²5*Û-ŽÚ? Óñ­UÀ?¥kNÃ=rÙ?©e…ÎeÆ?§ N)Àm/?ï"Ëwçï?'·^(Ën?Y¥úœfÄ?e[ÍFLb?‡Øbèy+?Ë£îHEU?둣â
,L?§à¨À|š?³?#VØ®?Ÿ<¯òƒ¨©?°3½êWÄâ?šzç-6Á<?ïњœé?"ZÓùÚw?F$#ü.³?W]2X°Œ?œ«ŒlH?"ìáãé•3FGL J0203.6+3043@a™Wÿ›V2À=¢ê šª;À8Ký¥²¬À;3˜ÿ?æ ?÷ÃkQݘL@†Êò9¼?ÿ?Ü+zÝ¿Ô\ãÐõPz¿ä+y@nì¿äAÜÕiº•¿æ{¬F‰@AGNbll?ï×Ú®D*Ÿ?mÆ?h«z?Hªú+'†?K'ì\žš?pýI˜zp*?k¼﬍P?ïÉ-{ȕp?xŒ1y|©?Lf'B/Öh?V3Máñ?wÜqÓoM?u]°¦ñÕ?ìžäv|áç?¤RŸ ¥NÅ?¦ù¸…çY©?—,[9àú?¯J‡Ø?œª—¸øêN?ïîÊE=?h
ð;¡iv>öµ¨@›†?
ªÞu]ë?axª:›£?gÿCžòa´3FGL J0204.0+7234@`î¿eÛý@$ô "AÀ9-¯d9ÖÀ;aâÔvz¿ºýŠ*¡ûN@,F|ç_@ÅÈÿ¿F¿ÙnQÂ?€¿è‹ÌŒ¢å¿Ü©ÁÕwì ¿âê%Š(8AGNbll?î lÐ~.G?´7.–˜,?w¼æ+°Ú?yØ\ô¶?«–&7¥b?³õKB]î?íÈ[QéMG?³·È5Ÿ?'=ñýŸ¬?ƒ#<¯	?®ù{dëÛ?±Æ'†'Ó´?í#ód*Ï$?£úª¼E"?—$]0ÛqD?‡ KdÛàs?±M'rª›? é\KBN?íSå_†2N?›ªmAŠ"ª?gKPÍ»Q?aõì'r?´¨¢©Gÿµ?›ªC퍇Ú3FGL J0204.2+2420@aí" ³Ô®ÀAΓ [TºÀ:ÑÊbAÀ;șÌÅ@¿Ê/'Šxá¶@
Óú=ž?ü­ŠÒS?ÕÛç·èË¿Ú."f\‰¿âÛ@°…€?´ïA8P÷AGNbcu?ïÀãé%f¿?}Ttí‰û?=úh@üú$?=yÿùðÁá?}®dé<е?|öâxÑIÊ?ï¼ÕÜAÐ&?x§Œ]©Üx?J¢Çì?m\?PpA›?~@¸áÿ8?v­(Ã}
š?î… ßkÿ™?Ž,Xpûô?'èDZj#(?'µGcþ	?sŸ¸éÀ?"2ýuk¦?ï^"'0;?‹'­ûN³?3—åű*Æ?B:öW¡Åõ?"ßuC4?‹QZi3FGL J0204.8+3212@aü–þµÀ<%»À5ÖÀ9F	ç	ŽõÀ;åŒ·3?ÞÜ~¸@!↝h†@Ž—?w9G¿èð+Ña~m¿èz—U'пïÿì%úÝÏ?ïùqæ¢5õAGNfsrq?ïâÅō;A?¢ÁºÈù©¸?iÀc&V9?¢Ãëø¶û¯?;κct*¶?:|,´o»?ï;°¾î1?eøŽõ?bçªÜóÜ?€»us›J?"+Yå6†?–cˆqP]?ï.;ÊÎS?Š±Àwþ~}?ƒýã¿ù¡?w‹¼'B†?•ÛV´Æ8—?…3äÙðú?ï½o‰.ä<?†Ò|ç%R?=ØÖh?[Vz™iîD?wýçŒ5;?†2Öú[3FGL J0205.0+1510@b€ºÃ.¾ÀF	՟Ú%{À9M­Ûoý¿À;¦G'ܾ¿ñv8;/ÖÝ@± üÏÊ@= v­†¿æ•'¢)`¿æzò@"‡Ë¿è*…ŽŽ'n¿æt=IaÕAGNbcu?ïù‡&2(?P_!Üt?+GâžÄÝÓ?*S='¿Ö?Dã꿆)ó?LÅÙ:'€Ó?ï¾/ƒ&¶'?~"ŠJ?F'4;Ī\?Q.Îõ|ÔK?~÷å,!¶?|	Š®}i÷?ï+¹ôrJ6?ƒoÕÐ.û?}ŸŽ6µf?jSτdԚ?" Ýéé?€ejæn?嵐àcE?'ÑBë˜?­â~4E·?%#†(?† ,:ªÆc?'¿WD#ç;3FGL J0205.2-1700@gB¨€QÉ÷ÀQ‰ÿ`2o¿À8ºyà–®-À;¹C'&?ëÉîóµ'>@F‡7¯D@c¿Âù¿æ»§[¬¬¤¿éËÄOr&¿ìÁ®Û¿ïþ%Õ|ž·AGNfsrq?ï÷ÃÕ|Ÿù?På@N¥?@#*|Þ1H?DoOiè?@͐¡ì†?F+Y…1Ð?ïµLB³EÀ?'è3Y?R{E(Ó§Ð?YاKN#?€]†®?@Vµë2?î³iy@D©?'aä‹â ?–ô'….?ˆCÐøւ^?"Íãtåœ?…TuÕ6â?.å?'^ßé!v8?YõÓR?e
b¨=`?Šºç#$?¿§"ˆÒ3FGL J0205.5+6448@`VþKZ@£ÿywÀ7¡Û§[#<À;»·Ñ"?ùhÎÆ!7@ú˜Ê¼§;@¦Åæ(¾e¿àƒQé3$¿äŒ–EYÚ¿çè-µè&<¿í
9äI¸}PSRPSR?'Qm/×$?"¿(ÄÕD"?ìFÊbµ±ª?Àˆs0UÒ?»DpWÏ?¿ýKÀwt}?UbFžà.å?t–!lÔI?êuÙ|ó?ÃD¢nø?Æóc\KØ?Ã;ñÂ=?ÆmOMŒW?ª"eV/:Ý?ãÌ´$£µç?³g/=BÁ>?Ê_à dœ?«*½þÒ?{Š[J{2?zºJÙßx[?îÇ¿.n?­%…5??¬2D:Ìi¼?«'‰Ÿ1µ3FGL J0206.4-1150@eóWŸ#FVÀP¬Å@'HÀ9Z&d׍À;ÄAvÂÔü?²dŽPvv:@Gµpå›P@¦½M¿ãºÞì<²¿åRÙr2ދ¿ß¸ôäÕ}¿ëM‹,T­èAGNfsrq?ïð6ÁA>?`cr	õV?4rÚ,êé?5'¿Ï#ޓ?ZuÇFBÆu?]Ÿ$Õx5­?ïҎþ…z´?y¸@à44?B¾ülÍd,?LO´ze9%?t`¡/¨ù¡?wÈòu¸¸?îêuÁÓF£?ŠèOâFŒ?‰d™+³°?}@ø£;‰?•þû0QÜ?ƒÍ¡W³õ^?ïì°°?b©p€‹>ôDlº`>ÿ¯eÎ!Óú?c'X%0‹p?bœ&NÀdî3FGL J0207.9-3846@o»'_ét£ÀQT_Ó¥.À:,x'¸ÔÈÀ;ü6'cDs¿ÔýÃw"@÷Îú¤vl@Zk@•ÇR¿ã[c$VeV¿é&çx¨:û¿ã¥¯½ƒ¿ì	i4àeAGNbcu?ï§üN‰ê?ˆlɏë?X.<q°4?f4³Jº_<?'û$î'~Ò?†L'hƒûz?ïZD{CÛr?—wș™¯ç?e¿àîöD?j{mj{ð?'ø›f³
?–'"\œÁ?îKõÇ!†?—I9sE™?—ìªåçÊo?…1ŽMƒgð?¢¤ë0š\?Tƒf[\v?îbcÒ؅Æ?›Šæ¢?g¹Ò±Bª??g‹×ƒÁtV?¨^%§cy?šùü¡³°É3FGL J0208.0-6838@rMÀÓgÀGy¾Ÿã_¶À:	~(úË
À;â½µÔì¿ÝÌǗ6pˆ@ÞXºla@]HÀŽ%¿ãâú˜ž¿çZ|Oz£¿â"Œ c¿æKõBÑz AGNbll?ì䈏
8?¹_Rí-'?v¶PÝí¼?­¦dâœ?·z0"Ïg?¸ÁKͅÈ×?îpAO?°€ ë'õæ?€b<YS«$?'¢¤ÁÑ5?¤ã`·¶$?ªa—Þð?íUò?²Í?œK¼ç—ž?–.éFÀ7?ô÷6R%f?¯Œ8þó%?˜ý÷"æ¤?íWnÉM?£l§ø?÷?rvvíêÚ?kÅY¡ ?´(•ÒÖð?£PƒWôz3FGL J0208.6+3522@a‡?'æGÀ8á݀y7$À:v¦—®ÝÎÀ;¾Â±(,¿¶ÄY'À@
F¹q?ûG޻⚿ïÿæƒhf?ïü™¬l¥¿ÆFóƒN¿Ý|æì™×éAGNbll?ïò»æ?XS^"Â)Ã?&´+1|˜?'W®7ð ?W²{ƒaj?WOoÂ2ù?ï[ã,Y?–{Ǐ>ž?u?7'kL?ˆ
¼¾ïë9?Ž›]ÿ`?ŽÉÜIY"ä?ï 'ö$©°?ú,Z3?€›ã½NІ?i|ñ ôO{?"­\Ãa¯?~IlÈñK?ï\'IÙçF?áM~;‡?s.ªvÙÇ?pøÇ^íˆæ?DXN¥€?¸ô³ï߀3FGL J0209.4-5229@qeˆ`VíÀN_JÞ™À8"Š¥àϹÀ;¤TÞ¿¸ýûh@ꨍþ0?üÊÈ`Ví?¯'®\¹Y¿á#}ë麿Ð*.QÌüH¿ÜàÏT!ÑrAGNbll?ïùÈJ5?cg£+âߑ?fµ ûC?ˆP2Œf·?J-DÅV?cT#B:OÈ?ïÎ
1(C?{¼b뇹?E"lhží?P:$ÓÎ"?vD‹ÚX¿?yþ²†"Q?îË&ÁUë?'­ÝH ?ƒM/z;î½?~=#멋?œô$¦©?Š[¯¯?íé%_"¶Ç?šïý·1Ç?(³Gg=»?1ÎNÔªG·?°ª{Ɩ'?šâS-Oð3FGL J0209.5+4449@a&uûmÊÀ/Â\ÀË6ËÀ:BÖ?<VÀ;ÒØ|-x¿ä©gög¡@Ø j™&?ÿ'DÁ%#ѿ߃õK$¿éw";ueÌ¿Õ²«·1Æ¿Å͚xÍØLAGNbll?ïóX…†ì ?`´ðÔåÝ?û^û7êI?jBۍ˜…?X??tB)?`jOº'n»?ï¿ô#º?€U³H–O?SJÕ à‹û?Zeùny?{39	¾®?}ÉËæÙ?ï%‰²´"p?ƒ}£ÔÅø®?}a³&$m/?nÊ‹‡û³?"ö\ßäV¤?€ÑKÅ!Ø?ï¼øÛ;úE?wã"Ìb?"ŠÑÞH?v<¾Qct?€±5¦/ìã?w
«Ñ¢3FGL J0210.7-5101@qAÉ 'RTÀNâD?Êñ*À7²¢
¢À;5ʎ.+Œ?øêò4:o=@úJ´Y9@»zú;¿ât}ŸÔÆ¿ãÛb¥þ¤¿æéãC!¿èDUºœž‡AGNBCU?ïÝÆ>-Ï?pŠî¹¥ˆ?\U†â"Ž?[\•Þ#K?dóè??k^ç}j?ïÖW}Ԍ?uŽeÑÂÔ·?A¦¡•"w?K¥tq›ÇU?rÉ#M?s¦»ã'BÐ?îœìOÔí?Ÿìaf~l?¡O‹Vm·?—¸R³ã•?œmKÉ)ô3?'u£ŽÀ'Ý?ï󑊴°'?dÔö
¾
â>ú¹áóG˜°?×ÏÚKŸ?XrÑÜß?dÏ­ifïO3FGL J0211.2+1051@c}sÉÀG®ÀGƒLÀ7Ƨf
öÔÀ:ì)é•ö?øf)Kf†@4ïY¿Ž÷?ÿU¥`ÍX¿Û\™Õ9éí¿ä1øh1οà÷[s:¬œ¿æ.â톼ÙAGNBLL?ïÑ.š-$?t¾hâ=6A?&Ç¢ü/·?$¦ÒR=Á?v²z¤Vj?t£;5Ò´\?ï¿BÌÐe?~ÅQëZr§?K«'‰iø?T)»ð?|éˆHj¬i?|gzN÷u?î,÷u™âÓ?Rj¥ñ|?'ð
ë3̶?‹Ëڈ¦1Ø?¤8°Çìz?•¦Ùó8"?ïœ"J9Z?‡JV$}âS?'|¨úï?9ÚÓ#Z'?ˆ¡hKi½S?‡!Y|'"3FGL J0211.2-0649@e3<`ŸÀOI¥ÒÀ:wò
ÎõœÀ;ò¼.ÿ?ÒIWMöÁ@ÿsì@Ë·À A¿Óì¿þC¿àÆۘäà6¿ÓYú6+Ný¿î‹o5~"VAGNbcu?îL%òG/[?«PyЅ™?£kÁÃÛ?¦õßy}Àþ?J0g$½?'ùìÆ Š?렓åŋp?¿l\É/+ ?©ßÎ1Ï?¯……
áå«?¶y¸ò9?´Ñd@'¶?èͳþ…7a?®÷žDr¾?œÓ#Hg'?©§2&ªBd?´X¹ÅEuÔ? òкƒ?ê©èSkÜá?¯×XœÓY?¡îl‡Ÿ»?ž‡KJúV?ÀÜÑ?¬^šÝ
 3FGL J0211.7+5402@`Ԙ€"åÖÀô'€—†À9¶^®@¦À;DDЩ*¿ü^øáӚ@
»Õtç·@‡¼à²^¿æyüàÎü¿é´¡¿¥>`¿ædŽŽ½ad¿çŒ
IYAGNbcu?í›/'©/ø?±RÁ¬qT¥?"t.ŽÃ?žùƒT®w?°˜Ґ®Y?®3MPÿg?'F°j?¨©P¨gߝ?t&LÌ箆?~Ȅ¹²ñ?£€cñø…?¦Žk¸×e?ë"Ä2‰(?¦¢ó9ñ·?¢ÂӆÚº?SÍ_Koà?¹øt¨J4æ?£-¸-¥?ívœBÞK??§§8˜"©?B$Øóf!J?PH-YÓÊ-?´&Ô7&Ù¸?§†'D§3FGL J0212.8-3504@nOЀ¶sÅÀQ¹¸!ïÀ:f°8AÀ;êTà,%"¿é#äV‰Ø@rå$ÝZ@ã矋öï¿Ë—pe~ñ¿è½VÃcË	¿Í'$[:¿ßdGKݽÐAGNbll?ïöµé<?`IìùÄÑ?×!-21?œ¼`]½?P¸€[uÂ?`3Î
¬z?ïÆ¥GùJƒ?XšÆ Ê?FçPdÂ?Mã÷,o?yí?"°²F?€0﮲I?ï=*ªæ;è?'{Ìòµý&?~klQCÔ?pîã%+üY?¿ã$2?}r;荨ß?ï‡S!ƒÍ?ƒ¾QÚ4Y?ï†MΧÇ?
lÈh"Ã?ŽOqQ>B?ƒ¸ÖŠ"33FGL J0213.0+2245@bN¶¿DNÀB,Ì?ß À9L=Ÿ¿™À;ƒ*¯ÖòÀ¿ø9§v@ò3ä‰@Éè <öÖ¿ØɄ\µQu¿â\û"+7ß¿æ'Y=çtÌ¿Õ$olZ­\AGNbll?ïUZM±í?˜ìŽÿ'?s9)?µm)?y¨vW<?†l\g	?•²ðÈÔÉ©?ï³ÈLµƒ?äñÀÖ?Ohý³Ýká?S=2G?H~"È©?€©;e£ëd?í$³àP°ˆ?Ÿ¿°ŠQ?¤\ˆäØ_Ý?"úL©·j/?©X9—‡?"ný­u­œ?碌#l©?•aùQg?&ð1.Tí?7ʀùÈ?Ÿ½ˆ9XG?•O¢ñ´T3FGL J0213.1-2720@kJµa
ÜÓÀQöÛÖÀÀ:ØU½¡¶ŸÀ<†Ï'yë¿íòcއñb@òSDÀ@µ­S·ã¿Ë—$¹¿¿éª"‡Ð³%¿Ýç'/xú¤¿º)¸[â»AGNbcu?ïÆ,ьY? B´V>ž÷?eÚihHZÀ? 'qÚæü?qüb…Ñ¥w?pÇFnAI"?ïË©Í
'?ŒiáwÊe?E¶ì%âß?L§"qg?wtŸ¾|ó?~+îÚ?îT7µ±w?"q÷
Dl?'"©½]À?ˆ"
kpl"?¡r¯Ð†¹°?a+AÎ?ï®cÚǕ–?€sY¬(֋?~¾f!p?Õ¬}Ìñ?"UŠ´xÝ?€lÜS§Àç3FGL J0214.4+5143@`øÈS'^À""Vßà¥ÈÀ:'º'GmÀ;²B@p…?Ýóõ°›¾¸@ӈþ–É@Uü?V,2¿ì=b\I4°¿íeÈ9ü6X?ä)¡¢¾Ë¿âp6,·ÄAGNbll?ïëê€:†?p×Olàú?/óðéz,?NàtoZ6$?báÖq-×q?oŽÙ'a?íè×h
¨?¸iöszAü?z¸Oà.È?"|<#üm?®…Æ¥?·†àSŽ?îǒËó·Ý?"O».Ü?€ï'Èï:?s@s4ó´a?ž•Ýu ?'	ï6P
?î꟨Öþ?¤u?1—ò?7'ϕÃ?Y6ìï]'Ó?¡0vãLñ
?¤rLÁ'N«3FGL J0214.7-5823@q»O?Ù3ãÀKØ'tÀ:MvÁ'}À;øшp¿¼ƒõÃf@ÿ/[bQ@O@…Z¿çs»
²›¿è'Í–ð¿âµpŸÐ?s¿Þ*x™Ä·ªAGNbcu?ïï™x\u?€Grƒè=?CJò®6Z?ûGƒ–?W~§•ï÷?Xbd¥Šn?ï­†¤EŽ?ˆÙªØŠ?S÷焁×_?eI@¢Ÿ¢y?':af^a–?…k1´¼_Ý?îápX2×?‹N®ZL"?û"+0ã?mG¯f*(?šÔ+d'¼£?†ë>Š b??ï9j(YI?Ž2T—S¯?G8e.öZ?Lñ?E¸/?˜©;Ë_I?…ï€OF3FGL J0216.1-7016@rO}ŸÓo~ÀF—€"ØÀ:)ݨ½#À;äsùÍ¿å²Åz'ƒ@8"IÖã§@…A¯ó£¿æä""Ðÿ%¿ç­ëè	Øá¿ç:dUr«Í¿ÎaßÆ$@AGNbcu?ïäòæmí™?pf÷slE?NêÙØê?XJ@^WÈ:?cRcâC?k0]z<k?ï°Á…ÝoÕ?'roº?Oš3wß?X},ÛUã:?Õý¥l'?,ԟÝ؊?îÝò1aw?Š	Õ]|žg?…I2O`f?sãXj2?™ Ñ©mã?"¢w¯™pË?ê0'?"9'Xv;u?$è:é7Š?29ŽrpÒ?úÙÏr¡?"-筞63FGL J0216.6-1019@f"ž²gÇÀO闟ÄVÀ:.\|ÙÀ;â$¯â±;?åÁ&5ò@…¿1¯{@¡NÿÂmx¿Ý¦ë®±¦"¿ååënù\ù¿åå'Íò‰¿ïÿÇ|ÆAGNbcu?ï÷c¡t?Z­Hê~Ó?3·ðÜ©{ª?7I¼W»ê?H•ÁBò¯?XTÀÜ|;?ïTa"¾oP?"G7•§?macó(ñ?q-Cø?'ǯE3°è?'*?Fn?î{Ò¡kn?•9+°HQÓ?œ+Â1%•™?Òƒ¯ä¢+?"Yåz¬ü¯?"çüIÖ£v?íäSÿ¿d? –ep[³f?Œï£@¸7s?ƒü0È·€,?ª~×?Uûä?o¤I3FGL J0217.0-6635@r%/€UûµÀH1" [TºÀ9 vö¢½À;±ù‰Ä9€¿Ùß-#û@…TøØþ?ÿ®Ó_Ž¿á
WÍ,ª¿âµ‹ñ¿×ôöí1Ç"¿â_O_¨uïAGNbll?ïöu,·è?OÙ6PZ²K?_ìÓ_k?r¥o¯Ã?Q?§Âùý,?N/,`Úr?ﱎkß?€:§]Ï?P˜v2¾™]?U ZÚ*å?¨ž°fš?}¤0| S_?ï`d Ê5?~ Õý_Ã??wºÔ…è?iõ9Ç¢@?Œúc0:?xú³¼»?ïFiu÷ð?…mK4˜#?0ñ‰OŽ
¾?3'Ž(Œéô?–ïõÞ?…>§Hÿh3FGL J0217.1-0833@eÎWà&EåÀOB:`NqÀ:^XƒNÔyÀ;åú÷''ý?çNáAsì@
F`·{@£, šTU¿ß}Z"õ?Þ¿ãl³vS]¿ç‹MF¿éùWÿ½²JAGNfsrq?ì¨Þ´:ñÌ?²ƒŠÎN?¥ì,gLt?©C½
^Ë?¯…èUÆÇ?ª5Äo'´?ìãµ-qÌ?´ý.D¬Ä? ;öRîߖ?¢uxDû4?°Ä[n…æ?­ÓöAzµ?ëuÂ&: ?¥ÀWßùj?°_¡ñkX^?œÄIªÈ?³òLނҝ?™gP;²¤?ç^nS)*?±ÄÓ¯nL?»˜¡~…Š?¨ø^ÊGøI?ĹõôWd"?«Çˆœºè3FGL J0217.2+0837@c"4 -œñÀHQö¬m²À8Ï}š_'7À;X}ÞR0N?җæEï£f@&âÙ(¦@ÍnB¿âSï¥X®\¿â›^HhW¿Ûx½­mc¿æáT~\|XAGNbll?ï÷·¨€?KG½C¥ýþ?PËWŒ¹?
'1ضÆ?OFo›­?JüµÎ-?ïÄZá?z+aADÑ?HuöAfm?PýºLÝ-?zÄ90b»f?w×:4'µ?ï2ª× Ìó?''-ôõíÁ?~TÜÜÐT?q ék}ð	?'mä²LÅ?|m,|@5q?ï±£µT®?='§Â?ř6ÅÞ?u•™ã9?ƒŠ)‡xfØ?+·+[œ3FGL J0217.3+6209@`™ÀµgU?îÆ)ñkÀ8yÛVÓKlÀ:­´{/P@îcßxv@
Ç`|?üÌÄ>]ß?Ø%‡P8I¿çQk"ôÝÉ¿î݆þâHµ¿æËW?4¦ÙAGNbcu?³Cj/ÜÑ?‡"ci?Í(JŽýŠÉ?Ì(M§²Jq?èv†Õl="?ÌSÀFِ`?ShÀ•†x?uGãvÙ:ì?ãSõÀ—|?ÎEaLCf
?ÙD…:;'?Î*¬¯C¬ ?Âê¥ÛtY©?®iËb›µ˜?ÔÏB¥Ð?²ªè,£z?á8Ç!–®?¸zRÂ.eé?€Ðþk؜±?v–£?éãb憍u?ÄMßñ6IÖ?Çed(@_?쁩æf3FGL J0217.5+7349@`§Ÿì™ò@'ïÆ¡9¡À8šÞ>åÀ;_Ae%Ç?íxNµ¥@ì؏ù‡Á@BBàzS®¿çÉÍ#½R¿êv,g<$¿íNÀÉD">¿ïþ>F./
AGNfsrq?ïð¿_ç:ö?díjû"eð?TJ¼…´y?^ÿ(ûžÂò?DmXðÃ<?Oê`âØƞ?ê+îC˜Ýw?ÃA¢k¶¯?±ñd6ÝDÛ?®¥nÃM:?¼¯)¬[Ïd?¾åS®@¨	?íÍ÷蜄©? zƸa?¢ãöò¹"¬?•§íó¿ï9? <Šƒ~0Ã?'Z¸£Ï°?æ½ï|´ß?½PÔòÄ?ƌGÉ*âÛ?¹²Hš?¼÷ôˆKW?³‰,x²n 3FGL J0217.8+0143@dE– hUTÀK5[ßú¦ûÀ7̄eTîoÀ;"‹›˜?ð­¬
µe¨@A*»?†©@‹ jC@¿Þ›Rú¬a¦¿ã¢
ã%§¿â˜rÉ\f¿åè×}æñÍAGNfsrq?ïïú¦Ð^?XnAÞ>D?0#ðn:I0?+^pì6k?\¶C´Lí?W°Nå´?t?ïÍ<ïÈȂ?yãl‰‡?E¤V£_Ëã?N]K:`H?v¬ýG/ű?w·	…Nԉ?¢Ž?"-46'
(?Š¾ï/¬îº?M«[$nò? ur9ëã*?'ÈÈü×?ï¦Ù5	÷?†©K»¿ê?!ﲚsB%?*ÄÙ X¹½?†óó1õj?†ŸBø´¾ã3FGL J0218.1+4233@ap‰ßrïÀ1² Ñœ?À7Á¿ß~€9À;
~gäì@ˆĆØ@'Mp÷@ñ†‰qƒP¿ÞíC7À¿+¿ä_rÆ	ÿ¿æS=nj@¿ëöDyùã~PSRPSR?~âÕ`Ò^ç?'ƒÌX\¥?î¡M½°
?°ðm—DЋ?¤)x
³\?°CÜÓ\IM?tú¼Í&½4?ƒäkÍÞã|?í¾.³<ô?°'@ê<ˆ?°À2½"¬"?¯H
	æ1?À Hz9w?«IúN?çÞ3Ÿ?²æÞcA¥'?ÀféCgdW?¥5¿RwN`?=ªµj6l?x·Zöm?í'XåË0u?¤sF
l
?±Eƒzù5?£]ºv"â3FGL J0218.9+3642@a»»ÿŠ;À6ì¡`7x<À8Û§¦¢–˜À;Ccf×¥n?î3·#\m@‡¦ÞP­Â@› ¿ã…Ÿ cš&¿è…Ámüg¿æªÊo‹Q¿ïÿ؍ÚAGNbcu?ïéC£çÛè?cCAC¡˜"?S{™ºw?SQEÚÛ£}?YývA%?\_é{DOe?ïœÍ3IU?‹ ˜í»" ?böûŸ¡1B?l{WP»èK?"ôEÑÞ}?†€MåxÊ?îjÐúÂ?'P²älÍ?›?ҘÐÔ²?ˆ¡z½Â7¹?—f-Öée?…©y…eÊÖ?î¹
s ž?šŸG–ãRÉ?pŒ!ǒ¨1?qȵ
÷ûµ?¢]ԕÊK?™8†NYú¥3FGL J0219.0+2440@bbÇÿÞrÀAGñQçÀ:Oá4bÞÀ;ÀËÈÀΒ¿Úo3˜@^¸»F=?ý¶ô ü9w?ï¿J£!¿åo7ýr\¿Õ	äEöj'¿ÞšR=ÜÑÊAGNbcu?ï÷+*êø?Rx&8®gö?ú!–Ê·?G¾Ÿ¡Ö?PYZ‡övÈ?QÎÏü~J?ï¶ø A*r?{‹°ÄÊ÷?QŸàSMŸ?Vg²Åô?€ ãóªù¦?yöG҆"?ïCkîŸ±?€]øX¶m?}5LæäE?jªý£!>?EInòQ?z2…ö^úx?îë/¾e‰?"Ax_å6I?4…6±{?=YFlñfV?¡'9ù­z?"!Ë¢]÷N3FGL J0220.1+6202c@`¤4_½Œ?î(ê@6b#À8ò=)HÏÀ:FÁÅ1ÍØ?ôܽîbž±@>jÉÍhÿ@\[ÿÛ¿ß¹¿³4¿æà± ÷[í¿æé  0ø¿ïû†ô{gOTHERspp0?_ݤ³ë?a"©m??³œ¶‰f?»«`äèv?í|÷O+z?»ïCUC8¨?«h?óšˆÐ?»±àŠª?ÔL¶ð]?LJ#@¤j
?ä#;%Å_E?Ën9c"ê<?µëf‡–¢? o5ÔE¬?ÑñŸŒ¤L?³¶9WÂQÃ?äIÃiÀ;?µ•ïò…?³X~­Â¸?®0Ûp«ÎM?ÐÐEˆéÑ?½rdxw{?å,͹EÒÁ?ÁQ«àøÖ3FGL J0221.1+3556@aÓjßqêÿÀ7{/à˜[¬À7œë"aq4À;
.óŠ§¿ìc²‡QB"@Š|p>@A(ƒÓà¿ã'›ê'ì'¿å¿aC*»Ú¿áùx¸‰°¿ã£ˆŒ<JAGNFSRQ?ïò3&±
ü?c¨ñozA?,PHæß@?<d>®Þœ{?X©Ç-?a<߀"A?ïÏLZ»ÒK?x]g4™I(?O:\óMw'?W°1Þ̎e?tr‡­+º?ukôŒÄœ?îZ!¤éúx?˜0ñá—À?' X€Bü-?{·Ts",ƒ?¥ÕϑO™'?–®"÷+)ä?ïë|虘Œ?f&N+á4N>ΜZåD–>êw…s »™?d{pePºü?f"/"Œ¹3FGL J0222.1-1616@gÉ hUTÀP—L?ß À9|ÙGdCÀ;Ê+÷Տ?´Æ;'õÙ°@˜Hí¯›d@ÎñŸêìs¿ãìå5ú7ê¿èˆˆODa¿éënÆåµ°¿ß~ý<'h´AGNfsrq?ïôêÇØ?\ƒ FLîX?6îÓ³üaÎ?8R³ý˜Vf?RK=q7´?Z(Ù¼{§_?ïÃ؍…:s?€³ýx,AZ?J£s¼Þå?SºüiE¿u?z¿JÛë*}?~N0²µ.¡?Z?†|þ‡?€™´¸ës?sõ´€ÑÁò?"*~"ØHe?Û~ÇÇë?ïx…Ii?"âÿÃÐ?R.Ýðà?T'!Xänc?œŽß'Äý?"­õ{y93FGL J0222.6+4301@a"Р+"À0ÄZ&–mÀ6]<¼HñÀ:
©yámn?ð‰•*6¢@$}õÏ$–?ýTÛ+µ:Š¿×>5фRÇ¿à¢L¢V£¿Üa|…Z¿ßCb¥ç…¶AGNBLL?ì
ö^|4?½òcbû|ž?S+{®È‹å?WPóöC?¿CŸ8ü/?½Ï¯'6?ïÇmP–"?}ÐÖb‡o?R™qjú?Y²)Yc£?w£Øzx?y}
O@¸"?ç%@^Î×?³1|ó¿1?—ÎO8v6?'wÎÞ?Ð<']pnî?²¦õXŒ3?.7åô?ŽQ374Q>ù?™š,"?FA÷".ø?E¥9lƒ?ŽFʲBÎ;3FGL J0222.9-1117@f @FA-ÀO¦ÄŸ×¡<À:h|°TÇÀ;Í8Ëùh6?"z)@…Ë[ˆ'?ý'ýŸþbœ?ïàMH欿ڝû'¿ã5Ÿ°E>¿Àa
ÂAGNbll?ïé½Qhe3?b]‰|²Ö_?2D2"	W?05®·
‰?cú(SY¢?a¤Ñ€hâ?ïÈăžpy?|Û£o›t¸?H'Ö2¯˜?Pµ_óËÍ?x‹ƒjqâ«?zìV=n1˜?îžhØÙ= ?Ž'¸âøt?'F¹æ\i?+J¶EÑã?›.ž*ñï§?"Oå¯:¬h?î̆VcŒ?™À<€gö?Or©.?\à—!g?¢»a"Ѽ¬?™e8Ą'ý3FGL J0223.3+6820@`hğס<@ãŸú[ÑÀ9¸À*'À;nºeÁû¸¿ûт"|ÿ@¼×ŒCp?þ£¿à€2ë¿èðÁFóµ¿Ø}j-4/v¿Ü¬è6ÆÌ¿¿ßšØŒ&GAGNbcu?ïß_]Ï%?tB}Ľ?DüòvA3Ø?E0îíTà?ka® 	?r¬¢d¶Ê?îˆÌȟÑí?­ÖĐ©{?hth•F?sÃãE/©?¥ëìõ ÷º?¬ØÕl҆Ê?îÆÖñ)°©?'±˜	¨À?"änãË	õ?v²÷`a5M?œ²êhäeä?	–+"+—?ïºøDÕ`?wžàR^š>÷®û¨±ø?Mï5ò…?6!0öœú?wšI‹)A3FGL J0223.5+6313@`¢Í œÃ@ye`,¨À9 @ŽÉ\À:ãPl)?ø‹×D;@uÊ\…!?þöx¥-K"¿ÚAøW
æ¿æ0NÃÌ6ê¿êö‡uœ©¿ã"øSIQAGNbcu?Ŭ'D?¾î›Éî³ô?Î4M(î+X?ÆÕý} Z\?ãè'$¤?Ì·
~k!?ҝÞæ?ÑQÉMEî?½eucê%ß?¼¥>-½?ãŠd|·Ò?Ф¬¼1ä?Û6D)Û·?µÔ9lºu?Éò×\øàX?°+H!M"R?×Ðu
Y´?¸	ޓ´D>?Ô>iúKÞB?¾ÞÌ7û
Ø?Î!ÖÅN?Ä`Ð5o?Ü°ª¢ô™?ÁZjÈW‰3FGL J0224.0+6235@`«¢_¦XÅ?ùáVèˆ?À9	"EœÂCÀ:lï­¢e?äc#c1}¦@tk0$µí@Íê€d?Øòtý¿çeg˜•›¿ëºÜ	€²¿âÑäÏ"£OTHERspp?ØQ<‹'æÁ?Í躽Ã÷?ÉX¥‰™ý?ÆS³ç{a»?Ûp¯ßLB?ÏÖ×s(?Ö샜Š"y?Óµ½Åw?³ÐJªüíí?¼ŒnÍ2ª?â´Ü[Q?Ópª.OïI?ԕSÃO5W?µýXâ‰>?Ç1|oT?+?± tx€?ßÑî«?·Y::¦˜Ð?ÏÁ‰UúUÔ?¿&OÙÛ²?³¼Ui»?°©ý"ùˆÃ?å›æÞT?Á§µ¸¯äƒ3FGL J0224.1-7941@ržq_ˆü"ÀBAÉ¿Ò‡À:ÏO^À;ÎïS	'¿õuŽ²Š×4@-#""±Ö@ÔÏbpã¿égØt~_µ¿ßÊ1%€±Û¿Ú÷sË:Ñ¿ç‰Äl'6AGNbcu?ï٫ۻݦ?}

í¨³Î?Lwè=3¿?Y'Rj"&Ð?o6*4ێ8?zàóÌ]'a?ï³	Ë;(?€V»ÅoÕ?P5¸² }´?V3ráœù?76Ý&N?~ëx"CÐ?îö¸_ê"T?ŠsŒáÑD?†u:."t?x'62ø+?–9e¤¤1?…õÄ?ïœÐ¤£žk?œ®­LQÆ?ò¯S:,?)%ðœÅ¾-?ˆ•–ñ¹¾õ?âÍU_H3FGL J0225.2-2602@jéÂ?«ºÀQA×,uªÀ9C[m TÀ;ÚºÌH¦?㧦¤¼YÚ@‹úÇ1€@NÌÀb†2¿æoû
¿è™›fÅ©9¿è<Éøj¿ïÿµððÌAGNbcu?ïýӓÓsh?0BÇ™s?'qãùéR?°"©?&3	Ö̝°?*KÎr‹?ïÈ~™½?zð\8K?KNÑK™>?Rî;Î;?x"†‰®ƒ?xk£Ú4º¯?ï'6馤*?'Þæ8ê½?‹B›øc·?xÙ¸ýØ«?Šï©ó>•?yÍE'?ïÈ5Šk?~›¥pT'¡?<8%!md?C3t辈 ?z!¹ ³?}֐>Í3FGL J0226.3+0941@cŤ p¸ÐÀGKÏ`%ÆÀ9'y…ýÛcÀ; dYEìs?êÐæ‹Kx@Aw÷ˆb@}±ÿlc¿"£úhóŒ¿èFwÓÌu¿ÓE
MXDÝ¿ëjò›Ø'
AGNfsrq?ïëœ,9Iì?eõ¡òXь?BÄèÉ(?EmHÀÓ°R?_¹ÅjCÀ?c8é¿+¹?ïkTÕ9ÁE?Ž‹#~a˜Ð?d8Aꠔ?ikØóROÁ?^PŠƒn?‹j4xÕV?ì¡Ågô(±?¥¡‰ò+Àc?ªÄS¥‡?œ{éØ0•?«škiÏc?š²±7ŒÛ&?îM«+Ê%¾?ŸŸòÕ£Ÿ?hþp7¡§·?k)âDʀŸ?©•f?㉺?ž©&ˆC­›3FGL J0226.5-4442@p_
߆ã´ÀP̀SÀ9ÙLvѵÀ;¶³ÑSDK?Ý~-Áü‡@É.²E?ÿF]7ãq¿âYËRE¿t¿è¯ÐôéeN¿´y´22hn¿ÛþÍýñªIAGNbcu?ïÎ-†œ?}Õíȉ<˜?*¢9‡äVÓ?*#-¾È?xîý_?}?¦3]Ö?ﳍ8êð÷?"Ø#ûïؙ?Pîpn ^;?VC5PIã?€þã·¶Ô?ƒ²OŽ®Äº?îüÝÓnUñ?‹U±hÀr?~xnu-ÞÛ?n1
˜<Ô?˜Æ)ôéÊ;?‡@ALpU?îˆ@a'õ?š–ƒê-ñ?DÒl9Íy?RJàÌfs?§+—°5ét?škºŒŒG3FGL J0227.2+0201@d¢æàé´ÀJh˜Ÿž–YÀ9¦Ž.+ŒvÀ;¨è»?܏?ÐSkŒ–@	éôZ@VOàh
*¿äÂÖxênì¿ã¥ªbÙX¿Ì~ê­¥¿èîðL7AGNbll?ë±ʶµ§?¾ÊÚ
>«?rX`
gú¶?rt=I9‰?À©1ÔÑé?¾"–¾Ýæ[?îZI–;ìŸ?©%ž}f€?‡\DH†¨?¤1†Øåº?¤"UŠ¯R?¦dùõ¯?ífÞ=ƒ›÷?¢ª>$îC?šŠlp«r?Œ
Þ9Ø
?¬LÕqêÉ?™Ê´©‰ÒN?ë¨}ÚèÀ?¨­œ¡L?€89jБ?&‰·Íÿ?ÀZˆ
òoù?¨n@3¤3FGL J0228.0+2248@bɸ!ïÀAq[ßú¦ûÀ9´Á"tŸÀ;–[ßú¦û?ã›@§~ÎV@z¯Èe@öÿ /Å¿àÄø5û:¿Þ*ÀžýAñ¿àøº04s¿ìÌã6àVAGNbcu?ïÁÞñ@*I?yyœ€˜?qžu߂5?qfEOՙ?kÿÑÔ²Š?j¹€ï¼O4?ïŠIMº5¨?ˆ7g¹Ó?^8db9v?c™ï\"o?‰¦ +gL?…†dd	p?ëÅ ^µû?§7Ä(<?µŸÏ†'Â'?¡ó"?¨n[©ë.?˜hgFâ¥?îúª_þ;‡?'—¿ž"Í¥?k‰X&dý˜?g¥¢1\?9ˆûkïr?'wÏËÜ
3FGL J0228.3-5545@qc²?î,™ÀL<—à[õÊÀ9!Å;ÞÓ`À;Ë®4[Q_¿õcl´3Mà@÷°(§>@h)@@6ý¿â}KÌ ñÁ¿æ'
ÏfÛ¿äŒR•	x5¿éö¥8^@AGNfsrq?ïöïØx0±?NÙ½õuò!?&°>£_a?%¬¹'Eí?N"™"fE?LŸB	þU?ïÖÙIóx?tÄ
qvñ?B"Ô=)F"?M'5:€úº?r@à~ÏD?ryÝU(ÿ£?ïÔº™Ù?‡0ÐÌbD?Ð|{	н?s×ÎA@'Ú?–*çÜÂ?'ÖÙ04Ù?ïüB±¡¡©?Lû?G~H¦>¦|tè3žÇ>½ñ"âU\3?=ß4¸~š©?L÷à$#Wz3FGL J0228.5+6703@`†‰_$RÆ@Ë# C+úÀ9‡½Q.ƽÀ;6O¥YÁ?½Š|lã@
òê|‹ó@ó° ™¨ˆ¿Ü@YM	"I¿ìP|V¿à*rހ¿¿ïÿ€m•AGNbcu?çÔÈ4˜?Åv"oU?'ž9º$?'aΐ+?Îy÷®Y?Å~ûà'\?à
`T"n?Д4UÂÁx?³™3`N£\?®v[+Ê%G?Ûò~êN?Ïu,Nÿ(z?æl
Í|ØF?±!ú¶íN?»ˆæÒe ? ¬'|³ó?ȋ"Ö£l?­Ú£&í?äp¡š®:À?·È§Çgœ®?¨¶0øNñ?¡™:>L`]?Ôö« ¢?¸ oÆ_3FGL J0228.7-3106@l«µŸôýmÀQ| À:Èá!§¼À<®ÎµY¿æ2¤[Ù3@d
‡ÃXZ@s`ù•¿ãóåVO ¿å'™³£c¥¿ÐZJÂN¢-¿Ý83<ZAGNbcu?ïØ7ä=™'?ž¡ VËYi?hÕ}–áWñ?ž'Û_ع?]å<W
0ö?f‹]P.?ïµÎÕÂ=i?ŽÀ6œ´(?O"ø-Cª?VÂÿ©R¦0?€š 1'?/{ÎNBZ?îs,®*o?"_ΪM?Š¯P˃K?'ÊXŽ.?¢9=xB?Ü¢´Ÿ?ï]Öe.4â?‡þ4¸©â?IRá0š?%ˆÐ­Ì?"%ê0'|?‡ökEªTŽ3FGL J0229.3-3643@n~9ÀëíúÀP̖üõŠÀ9&D7guÀ;ËW`9%»?á¹ØRUÒ@½º@N@Oß_¡{:¿äpô(G³¿æ"þnIM–¿èÓŨôe¿ë¸V5õ8AGNfsrq?ïõ€ê?\?VQ5®c?8{i§©¸ ??ä®a—Oà?M¾¢.¹&Ò?PL*v¼ñ?ïÔ³`WíT?výRïH¸?C°ÌHtñ?OºÛ[$ˆ?s06Jú·k?tË´Ñ(°á?îú5<›Ó?Š9*ü9ä?‹ùXö@}?~­u/Ô?'¼«ño†Ò?½rÜtPû?ïòËB ö±?d¶ÁVÅÖt?0ÕRz»?5£'9â3?Y½r7h'?d"!¹ÑÝ3FGL J0230.6-5757@q…E€<ÑBÀKL®¿›‹âÀ:Ç1Ç"háÀ;í´£á8?à _ŒúÇ@¬²£UÚþ?úõ@|òÅ?ßîCÐuº¿äÝþùDп⏃0 ¯"¿æ5²%AGNbll?ï—f'a¥8?®Ùqº½?Dr£ð"[?H'húgÍ?ˆß:ÝW©-?v‰ø{ò?ï±{Â+²E?‡;ö^Yߋ?T"['PÛ?lÕª¼sÇÅ?"ÉSz?'YõÙGc?îKÉæ,r?'­«æ¢?"†Ù
ˆÌ?…
Ê~ÃGî?¡õ'dx?‰\{@±Î?î^vöì>?¡k2P"»?b·³÷³?t;¢@¨F?¨íÁS? ÿ"¿à=a3FGL J0230.8+4032@aÓdÜY2À2€nÿ'÷À8ìÓXØjÀ;ž–"ì"?д>Ç¢'@z›Alo@e# ™5¿å©À‹Ôg©¿èqSlŽž"¿èé"¡¿ÝûžaTƒ»AGNfsrq?ïö˘AŠ©?OÊÕV´	?3¾%*gAd?1·7oÿ!?JòŒd¡¸Ê?L¦ô´ÓB§?ïÀ\—2†?~~ðØM©?T½èµV&?\>ž†'­Ì?zѹhM?{^e6ïõ?ïn‰œ?†^TF?€`CMŽ³?oàŽÝ£Ø?•'þ½iE:?'ñ}Ø8y?ïÛ:fx#?s[®¦~?îh¥¼;¡?_Ð`òR?r+©*,ý&?s>3·è˜3FGL J0232.8+2016@cýŸÓo~ÀBNº@NÀ:"7ÜæÀ;¦7¾³.–?áæ'²ƒ@)@Í$¶n@4ßxöâ¿Áô©Ú\ ¿èßiKaí¿æ¤ç¢Þ^¿¥g7"
`AGNbll?ï›ôôTé?†øqÁ&p?d'Õ§tZð?k ý1ÝÑ?ƒâ
€è¤L?ƒ·¨³›;b?ïš>þ"fs?ˆ¾z/w@?X)78Z´š?fÌÅ0Ĉ?†kt
?….±•?îY8Öãã?•qÍ$L°?"ÊuSļ\?‰‰~²zc[? 7çßp€?‹ ÀfG?îp†ó´(?Ÿ®ø3:Å?_å›ãU?kW'9»<á?§û'—Þd?Ÿ¥~póþ3FGL J0232.9+2606@b·žÀµgUÀ?n¢ ©XSÀ:Š°¬Ö)À;ÔîµTá?ݑwÿ‡o@.Ò¶p¿Ü@°ßŸã4ÿãë`FøÉ¿×Zp,>¿Ýc²£<ì¿ä§¿ zšŒAGNbcu?ïncÖíT+?'šÌ•²f?[)C_Ç?`iÑ¡¿Ì?'+OÁD€?ÂÀüÆz¸?x¥M…?¤—¡é˜?…nÈ_.£?‹D•£dÖ?¢	G"\? 	¹¶÷J¾?î?-ÍDAØ?–[ªT-p?WRAI?~è–ø¤œ?£áz[D?'Õ
ZB3?ì·g!=÷?£÷}É`?–`?æÅ×?'ˆVÁéþ?´¬¢çD^×? è98ŽÝ3FGL J0236.7-6136@q³SX"ÀI¦Ò?ÓT¦À8…´~êÂÀ;"Æü©3k?ç}¹ÝÂúw@äÇÉ@w:ßyø"¿àp°F%ˎ¿æ£ªGDk¿áހM¢A¿èˆ4X'AGNfsrq?ïøÆô›lÈ?EܬØÅ?$Ô;°?zõïT¡?GÜÆ=ûÜ?Dª&$
ð?ïÕW"-"M?uÿ|â\•?CIKBIS?LDT0db?rë
ô§ö?sÁ!ö:W?îù׉ËÒó?†Y"A…/"?ƒÐØ?(Ƴ?u>Áš;í?–Ü¢¦ñ>T?ukÎ
Ö´?ïýÍ<ú]ü?BÖÉ,x"">¦ÀV?aSH>¿¤´]œ¤-?1Š¸ðvW?BÓ:>R{Ë3FGL J0237.5-3603@n%ËßÒcÀPr¨æj-À9êøš°ðÎÀ;ªÞüz9'ÀëhnSp@®xù¼?ý»Ð@Ô¿Ôûè]ê¿ÚkNûï,ҿґ*2w¿âÞM[ä"yAGNbll?ï£yd¿ï?Ž¤Ç¥K€?Bk©äv?H¼&0ç-?…úõqÑ?Æ]éz?ïÇ+ô×Ä?"‡LlG–?G8ï(G?P«k\º?y‰ô^v9?ƒW£Í£Ÿ˜?îƒÉ<Tþ?'üú;¥Ïè?=•÷Cg?€ž‰¦0YU?Ÿ`á1ù3?‹o¾t¡x?ï¦ß(—?†Çnýb'>Øå ¥ER>ïã֛ê<g?†E"Qřë?†Æ)Ÿå5>3FGL J0237.9+2848@b¯8¾øγÀ<…'ßBñÀ6ë7OËÀ:ûìƒKy@6?çÍ@ h(,ºž@*%³Bâÿ¿áêÀӚF¿æžºæÎß)¿æŒ*Š¿ê½ucÚEAGNFSRQ?ï²$:É]¶?~–
:¤—?s…Më$?yÔ…Áðk?sh"°<
é?nyò '¾7?ïȪ¹³`?yMiNs?OB/£±+s?ZÈS&6šÙ?wÂ]2*I?ulÁ€°$?ì'yf¨½ü?§y*JE?°Q@½;£R?¡.8Ë'š?¦5èüٝ?šÓ-"¿g?ïöU¼cë?fÖ"PF*¾>ó$ÑÅ­Ú§?ÕÂ<ê3¬?SŽÁ@!rù?fÅèPZ'93FGL J0238.3-3904@nþã€ßÀP0‹À'¢ÜÀ:uå"m/®À;÷©4AP,?×Í/@Ð溉©7?ÿ] D-¬?ï÷½À"-æ¿âÕ -qþ¿Ë\6;ÙÓ¿ç8€šR¸AGNbll?ïè¬ÇJ?gU¢mºN?>…]Eö?Bñvz]ۘ?cƒM͍?e•$Äû?ï;ßùÇ£?š¬Ú‹èß?p«ìælpg?wLÇËJ?"Y¤Ëïk?–Û·ñKò?îºÉR@€?É0)8Ñ£?Œ¤ë¼Zì?û@‹1S?šT_Ùñ'h?†ó×wϋ<?íWK±ëXK?©t'ÓTÊ¢?uaÀ
^7Î?wp±Ñ_:Ÿ?³ï†oÿZ.?¨§Â®¹uù3FGL J0238.4-3117@l¯¬ºËCÀP•‹B¹À9XõL»šÀ;hœøɪÙ?Íè»q@ñ@áü]‰ ?ý^%y¿ÒúÁ?ƒ2¿ã
ù;H^¿Ðá¢Y(1Å¿ÖwÑýÅ­AGNbll?ïÖÚ±g´'?yE;í™?9†½Ã?8è>°oŽ?sîàI}é?xÈc4ôÚx?ïž~¹Òp¤?‹Î:ˆb= ?[C3>m_±?fOIA¡Žh?"÷ë#–*ê?‡È~…$#Ì?îfe"Ã%?'	r@_üÏ?'ÁoÒ#=L?^áV£m? ¸îʽ??‰°ÔÏãAÆ?ìSQË?«@œ}í#×?TZƒÙY<?`_$GÆÙb?½­
æC?«F–Îà&¡3FGL J0238.6+1636@c˜à¿]xÀCÏߦÄ%À74^¬]ÁÀ:¥žÜÏyO?÷³ÿEÅÝ@!M^|Y@…Öí¿Ý諍ën+¿ãÇoܘ&¿â6"׿æªÒîò3AGNBLL?ïۚC–°^?qeû¶³L?('Šü@?(%lêÿ|?qnIã÷ð£?qk¾f@Ô?ïξ÷" ?vW	–ÔE?F+VS0?R<GTÛ§?uیBT%é?sœ2Œv‡6?íƒêl¾¤?£Béü5@Ø?'W>Û|5ü?‰"š·±¼˜?¯¹ÐEú¼?¡H•âá)Q?ïþ''ab'?<5Ö*i,>­Ëeídé>햺꣧?&ºƒêq?;û·öV$j3FGL J0240.5+6113@`õ¹pޏ?ñada(ŽêÀ5xþ'jöïÀ:%ÂÐʈO@K4[Ò9@]Ë5ó×Ô@N
Óî$¿Þ'Q¦»Á¿åt÷ù¡A.¿æÉÀµg¿ëS?bk…	OTHERHMB?æ'ÎΗ·?Ʌ½Ã[«?ÆjOü'±h?È#¯H]
ª?¾œïX…ß}?»xL<i>?ÒàD¶l?ÒÀ%¿ùÞÔ?ÒôIJÝQ=?ÑYíNOð²?Û[	øW?ҒÀž€%­?ÜÔLå±?¹ƒ'—-aþ?Ö]ÄrµË?»å¾øÌ£?ɛßÓÞÉ?°8†ÈÄN?Ë8LÝD ¬?ãQ†äs?Þ>II½sÅ?ÐKˤ¿??Ô%G ;å?ˤ¹bp^î3FGL J0241.3+6542@`½œÁæ°@Ñu @&âÀ9>$'ýÀ;9ݾŒ˜)¿ð Õugá@{«Ý>@£Gßg¯¿â:ê«@FR¿ãu.å4'q¿á}.\'[¿Ôb³ðC/¼AGNbcu?éŽb¯åî@?Á<¹'È?†D"Kµ2Ø?'"€uþ?»?Èb+û¬óÒ?ÁnýÖk?ëÕ/¹	?ÃÌ/†×'J?ˆô–Žœ?"å¹
^f?¾7ñ@¥Å<?ÂNDq
ì²?ê¥Ã{H°?¬ž¸ò¸#b?§4wmì³u?'
eTr?ÁðK—°e?¨³±O*­?ì2"£@T?¬]Úî}•?W+ÂPõŽ?a•]>ªùï?¾«Þ¥©Š?¬+¼Œ	G3FGL J0242.3+1059@d:¬ÿ§ëlÀE¬×5ÜÀ9£YË8À;–¥€éŸ?ñäŸANSö@Xéçå¬î@N_ƒô¿ãÔ—m[¿å³{œGb¯¿è¶8¤ißË¿ïÿò"5£ÀAGNfsrq?ï0÷Q>õ?ž†J¨Òž÷?~9y̤&L?ˆ×qó°j?'R·eº?™¹ j¦§î?쮈ùªwZ?± ÷KÁŽ9?,CÀ÷í?ÖŸ×¬¶¦?³@§B¦<?ªŽÔ—øð?ìÚÅ(›?ªåÈ·e/?²@sŠÄ%?¢&^vÙ¦?ªVL—î?£'Ùø"?çÍïÎó.?²'ˆÒ?¿Š¬@ܘ¯?©¥ªFÀ8?Áz Uæõ?ª(Dcp23FGL J0242.7-0001@e"-@ªêûÀI÷˟¦#À9°}IúÒÀ;ɑ
ÙÝW¿å˜?	ˆÈo@
ΛzšOø@–€"û¿åsŸi½2ü¿äf>"z~¿åÿC!gÙ®¿×0T[¡çFOTHERsbg?îôçtñ¢Å?¦3ûd:+•?ˆŸhĵ?†—G#l?™€é‡šz?¤‹8ȟðt?ïÍÄ(ºÕ?ƒFê¥'úú?Q$¨ðt?cåtö?uTÁf"Ç?KÑ¬<?í؛ò}5Ç?›liK;k¥?™K´‡'}Ù?‰HC¹S³B?¥Ðf"kd›?"ùuü@FÐ?îãFiÔ­Ž?—iZŽõóe?N`¶2°É?QµPçŸ?¡R‰êe?—7¢–˜QŠ3FGL J0243.5+7119@`wL Õbž@$Ê· "À9h±Ä2ÊXÀ;r¨W¢~E?ڇKBƒ¶@}™èÉØ|@ãV€bc¿ÑÍ8[ÕØ~¿ä6Re¿âtÛ6ûrZ¿ã£üH‡Ð'AGNbll?ïˆo=Páç?—r«WÅ«?eƒR½µ1?h"ƒTjuG?ˆƒ[üZ9ä?Œ¢#f?íÐݜb?±}{öy{?'©Ê'5?€7|Ô@ܗ?®GÞL5"K?°Š3¦?î_èBµx?–"< ·˜Î?îe=†¦?"Iôko¼Ï?¡ŠIAUå0?'ÓMIJ/s?í¤šÈf Ð?œþöŠš©?€ôß3Tž"?w̐ á±r?°¼Ö`e²?œWþŠ	3FGL J0244.4-8224@r©óà7ÝÀ@ßL߬£bÀ:tÇR9‰À;Ă´zÆp¿ø•€Túe@¤ççÛF@n­ŸàÛx¿ëÚåÇÎü¿áwëøÕþ¿ä8_öhZ:¿ïýÀÈÐÇAGNbcu?ïÁǓoe·?ƒà­_ÖÎH?tðšÒ‡°Q?{ùÏÕõ;H?dW6ëŠé?v»N5±üD?ïmRRš?–B!ûÝBU?g‡GRËm?wa¹›Åð?ŽÉ™"óÇr?"²ÛV² ?ìÞ¶©ˆ¡?¡U±•‹?¬Ñ1õ¸?Ê?™áد"`H?¥M²Ÿ¯6/?"*I-ý¨Û?ïV²Ù?–|ÚqIš?\M•ˆÑÏÔ?m‰´³œûŽ?œPb¯‡¤?"°o>~~"3FGL J0244.8-5818@qf{à~íÀJ‰~¿ù³À:Õ¥¹cÀ;©ë-àãÛ?ғ&
ö4@
˞¤pb?û-í"Ti¿ç«/lìâ¿âˆÓƑv¿ÝE'"&?¬ùËÏ÷¥AGNbll?ïÜÎÍ®A°?vÄYÄÐã³?'ߘô"Œ4?($*0%Žô?pٜa;Ë?v'üÙªP?´€?{ed2°?HS'?O•DL;		?y³
»M¶{?y‹öjûËô?ï>.hËË9?"i"®p6B?|´®u^W?puÎe<ps?'
I&A8?€Ð'÷?ïr»øF¢?ˆE…Æ։x?)oÉ,›÷ì?>y¥%¾{?'u¡dæª?ˆ#¢ó¬ú3FGL J0245.4+2410@c7oŸËÀ?ȑ_8t¼À9)›«Â'
À;'ÇÖÃƔ?ðL"èÝy˜@JÃú@Mx@¦v pMp¿ä‡mÉqȿ稦&𯫿ꮇʅ¿ãä¼òAGNfsrq?ïõ+¢K6?Qm—•µ]¼?D—G!ª`æ?E•·ÜÙÐø?Fº/±øÇ?H×3º$ÀÅ?ïŒáÑvC?^½CÎ4?^iH¤š*z?bßg:†jT?‰,^w*d?ŽÍéÅ>ˆ?î»Iì3Ó?9óM?ênÅa—?t
DÚ·y?šÍB"î,?ˆ›Ò1AÔ?îR|#ç?¡§4µãk?{tÐßíØ?}=þ ?§i¤ñÃçr?¡1ÀxA>‡3FGL J0245.9-4651@p]_Œ¨ÀN
dàTiÀ7š¹y2ñÅÀ;F{jÚin?øeZ‡àß~@imãÞ6W@ÊA€h¿âißW=ÿj¿åðxô'˜¿è? Ÿ»OU¿éåb¶6;AGNfsrq?ïÚ~Ö/o?k€ Þ0Ä@?h»Wù—rÉ?cÜö秦»?Y‹£­òÛý?]ïÙÕÂ
?ïËýŒ˜Z™?yí"øH´?F~ÍÊñæ?PëBΎ¯¨?w1_út"N?wܳ#i+ÿ?îÏü¼ÍCÏ?"KŠ•b@K?'•
"¹â6?‡8WÃËÙÅ?"k]ҝ£Î?ˆØ 6c
?ï»ë2Ñø?…é«<­?7_]VÏ?CRwç8Ņ?€L°P—I?…Ìt]¦3FGL J0248.5+4232@bÏÃøÀ.—VgÀ9û07EçÀ;Ö4O'åJ?ê¿7öûï@
'­õF=§@T̀K¿Ç¿éê7§ó5¿ØtKR¿êT™"·v5¿ïÿتrýPSRpsr?æ!gbÚ7?ÌOoþµ+?ÐPB@×ß?ɦJh2"?«gwË£°í?·YlÜþs9?Ð5dÌZՒ?Çý›ʔÑ?á!16aÇf?ǁô&>MÉ?ËqÃ7B?½±à>õn?è°/<í3?­xÊÉŸ%?Á)üA»?¦2ºJôò?¸z4šúð? h –Àx?Մ¡sv¹?»t*ÌÛj?â©kvu#?¾Ú"§@?´¢!>r?¦1¯ˆí"3FGL J0248.5+6022@a¶â—?ç*‹_Ö:›À7рuÜ%/À:rgᐩ0?ÿXŽ¤ž@ÊÈ.›@Î`=Wyd¿ãââ%­W¿ä"Vÿ¸¿êµDøØnl¿ïÿšFçPSRPSR?¾äë@çˆ?½ÜmÿcPû?â¥È[2æ?͗¾¤m*?Òû4y­¸4?É´gz²kv?{™¤*)?›í€\뛾?ä€ëµ‹ìÒ?ÉJʌCR?֏Â"%³?É¡9éËZ…?ÊH>x7›?¬²½"0A¸?ގS3JÊ?´½^SV?׬ˆ­Á™g?³£h͙DJ?—Ož	Œ¼?‰I%ᓵ?è³
Hë
¢?´©6Ï%ôI?ÊI׃Þ?³
e33¥3FGL J0249.1+8438@_qåÿ£¹®@6my€žQÀ:
ˆÊ>}À;鯣ÇÀ$"Œ"xs@Ҕ%'_@,u?È¿ßù7r÷³¿èÞ X7¿Ñô²_õDK¿ã&rèÕÁéAGNbcu?ï÷âöÔ?T-Û,–«á?17¯>aÍæ?@b8DÞÂ?KLœ…~Ù"?MúV‡'d?ïžî+Fî?˜³‰Œð?aîIv?l(>åƳ?ƒÈêñ&¦û?—5uäÕù,?ïIŸŠí'?'Âߥéà¾?zL¹¥?p9;zAH^?IKà\æw?}¶à$`vÿ?ïî¦dp?b@j%h'z>Èc¾{J>㱃ïú³?aS–*·2?b=ßãä'à3FGL J0250.6+1713@cí€í )ÀB‡dàTiÀ9î&'d@òÀ;Ÿ_ý–™?뿸Àâo@v`Y‡?ÿ½±žÉj¿ê77ÙO¿èM^»Ðù¿Â2MD¬Wa¿ÖÞº_3AAGNfsrq?ïå²A@6|?fÈ¡Å÷7?=QK¾³/Û?<±'mµ?f£•Gó?ea Š¦-t?ïs‡Tõr?'ç
×?bØeegÐ%?q–±Ýj?Žhid¯P?m2˅S?î›ÀŸ±Ù?•š@Éóyw?ýªÜ­Ë?…V0c^–º?œ ò}³6{?Œ¥ñenõ?íá}q\?¢}¦[M-ð?`ߏ6ð?pL…é€>?°l‹ûnÃ?¢4ŒPœál3FGL J0250.6+5630@a[¦?šIÃÀþ¬@:WÀÀ9ŒEÅ.îÀ;FÙõª;¨À{èP¶Ñ¹@z<Cþ¬?ÿØրÂ-¿Þ\†öÅ¿èVF3HµY¿Í›Ý '¡¿ÝEX"ƒÅAGNbcu?îѤ
'.ˆ?¡Ð‡‰t
ð?S(›lsá?Q¨[â[¼?¢LÅâ³î?¡¨Sï»Ï2?å"ÉÎS¯?؞‰tTµ=?‹³i@?¨~Ü9Ö?Õ
ÞÈ?Ø74I½!?ìçûEo?¡ó9,˜ó?•ê"½TV?'ß·Ï'•(?³E$¡ÿ¦?žÂDÕNÂ?ï'Pj¦g?…øfõÛñ>։°×º>×ÐBNsQ?‹ª¿¼Å;Z?…÷á"æFì3FGL J0251.1+2603@c=X@žUÁÀ=ƒ?ÀàÀ9´üÄâÀ;£XãÆäU?ó³	ªx¹û@Ä;dÚö@J3q¿Ôö¥»][¿ÞAç«ö=‰¿ç{"SÈeE¿ïÿƒ€¨†òPSRpsr?ÆÄ ¨'À?ìZ°|³?çD‹Å?Ê™é\ýª?¹}ž¬VÎ[?¾ÑïM&A?¦&*Ÿ'Nf?§C³™‰?èŠÃ'Ö?Ã×÷µx?ÈKgO¤?ÁŠß­Úf?ÑU†@tæ?²ØnÅ,,=?àê‰Ë)"?¶Ë]Ã`W?É«ÕÆڎ#?°©+ e?·4Òò?¦VÝV›¶?é¼×ºU(…?µ'$Âz#}?ºäpd<Ç?«©ÏËB¢3FGL J0251.5-5959@qu€?öÀI¤¨à^z	À:phŠ'¿À<FJg,_?Í퉊¼
@еd¦GÓ@QÇߨ½¿É2Å&\­w¿äÍÎZýÆ¿áåǥϦ¿ïÿ¤D1LAGNfsrq?•±À©?"[±¹¾‡Ç?'%3ÖH0?Ž-Uè҄?tëÍz¨·?~[´3®^d?íÇQy"å?ªË$\Š?Ž\nå?R1‹qÒ?«óÁ<-5?¦sér¡T?ë"ÎôçT`?¥&¯‰®?¶÷¤Ú|Ž?¡ì"˜è—?¨ÓÕgÕÀ÷?"¶º?í,V×ó(ã?¤[ÿ!:(?"ùžý*'0?æ(\Üeã?±^ၚ? ÌÖ,ƒPQ3FGL J0252.3+3830@boaŸÂ¨‡À2ˆw"^À:[àíìEÀ;Ò¡áf·Å¿ðvĖrs@'¶YÃÀµ@ø-Ÿ nË¿ä'†#+d¿ë¦Æƒ»š¿æ¡«;W™ð¿Ð–Æ\˜AGNfsrq?ï
7?e…Ø`þŸ??Ÿts?Bów —ë?ZmËÒ?c=Š£iä?ïºvƒaì?½'¯Ñ
‡?W™Äߢ^8?`{5Sx?|ÞM![{?~øÉú•h#?œ¢mÓ?ŽóÆ pØ?…ì ·ã¡Ø?uÌ?ýú?ŸwüÀt»?Š/~i‹?ïÀ íÓ`~?w/UÄ ¤Ð?_N@{?ÑÞ.Ì?ÊÊzA´(?w)dó÷å3FGL J0252.8-2218@j7ÿyÈCÀOŸÿå(
À7–>Õþ¤¶À;"™.9Ï?ø¨y @Ò'{™ÿE@ª"—(ü¿àÃý1…g¿ä£·F4m¿æà*R—… ¿çcò:<AGNfsrq?ïÚ15ò¡Î?mK"AY€j?Z+‹‰¦Æ»?Vðãªë?h¹HŠÎT?hŒ^KÅ?ïÔâˆu¤ä?vkKÉ=ÕD?CZ~V'"¶?Nì¤ÝNm‹?s#kú]I‹?sï.©I?î'{¼?—¨ÜTóØ+?"«¶©—àÐ?+Üïû
²?šÑÓD_?Ž©>JÏ*°?ïíØÔs;?o6Á‡
f>ö̋ª0u?¨ß—ÆIo?aù'u"d;?o)nzÉ3FGL J0253.0-0125@fMþûôÀI'/`?Û¸À:Q¢xåÅÀ;ÄüÓ$Õ¢?ñŠ´(æþý@=s˜Óöã?ÿ.Î*L…?ïìóǞ Ñ¿"ÙsÌ+Š¿áê
ü™T¿æÅ&TŸáÕAGNbll?ìDs±3?»?mѸ2? ¸ál³I?¦ÙáQ‹­?µ'Û¬å?¶Sj³¸=?àBäZ«Ÿ?Ï$Ô[QíI?Ó'~±1ä"?ʎm¼?È¥q2íºÕ?À čFO>?ç¦Ò‡‰N?µb°¶ 'l?ÄVj{Q?°˜àz!yE?¿5ª–Í'?¨`‡Hæ?Ô35™v'?ÀN¡XIŽ6?àý¹"›Ò?ÃöL|®?â®~œ¤i?µ\ÎH®Æ,3FGL J0253.1-5438@q— /µÐÀKVK`P¢°À:iONóÀ<
Ñ@±¡¿Ëùî8W_b@½'ÐÄÿ@"°ŸðuÉ¿âps9ÕÜ¿æHŒ'0Tî¿æ"×½cÍ¿ìUaÀS0˜AGNfsrq?ïñìÈèRà?Wf¹âkB…?<³/ÿð'?E?{ˆç?Tù¦ãZDV?SVƒd"?ﺖ?ðlW?~Ÿ"Ê??Q6­J'?WvUª´?~g4µIϼ?z 'VÛé?ï6
 Ð'¾?…¶²£ÅôU?…kì@?wöÅ-þä+?«‹àô^?}£V­/Ӛ?ï°`'Üy ?€T…r'8?@ÄÚþ2I?ATásuI
?'æ^û1Ô§?çlÒ:D3FGL J0253.5+3216@bÞ>ߤ?æÀ7๿©Î›À9±€•Ó;À;*,ú4¿ø4w
þp@áܼ.@k@?
W¿å,¶Á6…g¿â
2Ì
¾¿äï«õøÑI¿"ÁjÕsAGNbcu?ïýw­Ö.ö?0¬†ÄGX?
=4cjí?
Ç#€¢\?0šêÂòq?/Q(Šò?ïËøâZ?y©q
?NÛXŠŒö?Sè{«—?v(.Gì.½?v6Cp¨?ï]v;P"í?'‡S×Փ!?zúz<Ÿs?q§RÏÈ,h?‹%4#¼´ü?zךsçÏð?ïýÂ2VH?5J*§Æ>ysZq½Ý>'·‹žŠü?1î<æ`?5IÞjŠ!3FGL J0253.8+5104@a¸ ٔ[ÀcßÎ\DÀ8´w⏬±À;7ÞUõÖ?ÛJg@C˟¦#@Z9€ª4q¿çEZB¡¿ç¥¼'—ó¿ç^†7Ó¿æÎæ‡ÞÜAGNfsrq?ïé|Ñ_`å?cI;$/4í?P	Þí‰ñ?Tî]ýîwF?\ü~T1©f?]ÒíJŒI	?í"9 &š?µ}êZË[?"Jù¿".?ŠmÏÅÃù•?°Þ†ÿEr?³T9!3"?î–DÕX1…?'©šY¶³?‹ôzHðê?}óM,(àù?Ÿ=(0Í¿?Šy`¡º9?ìÞ	‡ ›?¢¢Ó¼ú?'R	ðuþ@?y'þúj¦ã?¶Årˆð«T?¢(üøyß3FGL J0255.8+0532@eFð¸,,ÀFÌëÿ—û4À:L‰°îIõÀ;£´©^3?Ñ¿tâ!•@
€Ý°ŸÅƒ@Ž¹?|AÅ¿Úkk9É¿äÁw:ß@¿Úo/@h¿æ÷–<ËkAGNbcu?ï(d…Ä.Å?šŸ5¸ÂP¡?D'^¨xŵ?DÖRwž?šO\R6a(?šdî—]Àx?ï*GƒdíK?–akð-?o¾dA(?u³=ßl€Ò?–¿C=E$?"NïDq?îAlXX÷?"Ï<F"Œ†?ÍsLÝ@ö?€'§‰øé?£'€ÙkÐ?Ž*sٖßò?ìlȞ÷Jb?¢Á6¹<?xÙø^?uÁKê9і?»)hÄ+n?¢ÿåU8I3FGL J0256.3+0335@e‡y¿ß~€ÀG{íÊ»{À:;ëß·‹À;©ãiÇC÷¿÷YeqžÓÀ@
|=&|?þVE^®â¿ÙÉ÷9 Ìÿå€øiø[
¿ßaœ;¤4¿Û%¸«6AGNbcu?ï^ºu4`?šÊ€© â?6¡YWÀy!?8 ƒä˯ü?"Î+ôúm?šª
%&ÿ?ïºà<•ò/?€¯.
›ÙJ?LùEaÕÀw?Sæ`H,›_?~ð¹Ì1
?~rvC¿X?î~WdÑ@ö?*¥;AxW?ødÐJÝ?{¿9'ÓÁ´? œp~Ùo1?ˆAÓýþqF?ï/ÐÖõù^?'BðÓb?™¨j­mà?<‡Kñ?™øM}ª?'?ì>ºCQ3FGL J0257.8-1216@hsÿ¬*ÀLr 6×-À:¶'Τ=À;ߎ¿K
?ßғ»‰-'@WðK'	…@Òýßê5é¿Þfé=¿ç;æqÓEÒ¿è\+´d1¿è71¹¥A‡AGNfsrq?ïù»G+ë>?NiîKª}?1þ+d?8Ý%\Íñ?@×Á'ro?E&ÙR:àý?ïÇ-Kn¶P?|ònq~+*?L•Òu Iœ?TÉçêÞ,?x֟ùðÏ(?yá¡é¥·P?ï
ãdë,?…©Ùò@";?†:Ko7"?yčíÏõ!?"&xÛÆÒ¥?}¡àü¾E?ïˆ\ýïð?…ŠÃ˜äÄL?Kvܦc'	?Imן±?Œ1R¹ÔŠÔ?… ,éå{3FGL J0258.0+2030@cßdÀßXÁÀ@¬‹ŸÛÒúÀ9úá:B.À;{E	õLH¿õq.÷iÐ@'Ý/p…ú@!VÇE¤¿î[r:"U?Û¶æˆñ½¿ä]}«ô²¿Í.–Ì	ÙHAGNbll?ïﳨ
ij?_œ=gÃA?6ôÂfk
Ÿ?A_KÍÓ¨?ZÛJÛՏ?Y^,çE؀?ïÆփgje?y¶ˆr0?IIÆMv?TH™çÎ?ykŠ")-?w™Žàž\?ï
¥¸áÏ?ˆ!ڀXÀ{?…n	%Žfó?xY1N6Ô´?""Dl|'³?€eräQU?ïÊðßĝÁ?v•V转ƒ?e¢Viô"?+†¿×i?z	ù"WwÍ?v‡¾ËWn3FGL J0259.5+0746@e$»%_5ÀE§ÒàD²À9E<æÀ"À;qkI$6@?ÙzAµ,>@ÇâöYã÷@²v BÀš¿â9˜/¿¾Ð¿å?U÷i¿ßK|‹ýàÒ¿ìfçsI×AGNfsrq?ïÜŠnÑD?pív¼æß?C¥ EJs½?Rð‡~Ñt©?nø
Üò?mÊ5Ø?ï¶)å6I?€"û•Ö ò?Qµ9¶?\‡,Ÿ]?€>Ö¹«7 ?|؝ÙÞ(?î
¿OW¿Ý?›5'A]yÍ?œý@;ËÙò?')$Ιãž? Õjìž/?'E3"£?ïQ]5¡o?‡ŠösÊpé?B(…Òr?Aô1ÌuS?•LsAŒ?‡E*÷Ü5¡3FGL J0301.4-1652@i~à°¯`ÀM"€ŸÍAÀ:Yx°"À;ßÿê0Šâ?îöŠâáP@*³In@4`BŠê?îÊ«ÖÊ+¿â²W¿Úv¿ä¼G_°¿è$å?èÖÌAGNbcu?ï‹53èŠ?ô!³ón?ƒ³\Y²?Œ;)+]µ?rÿW†Y·=?rtÐS?ˆ?ïRY/éw?¼E¯»F?w*|å¼Õ?÷ŸY%Ñ0?–Õ*:ÉaÎ?˜K­"
l­?í"ƒÝ? ü›SLÿF?§Ô¿]Õ«÷?–y2Å?¦ÊøYú6?'¨¯}O$?êڍxɽt?¶yl'[¼?¨®ayƒ<"?¡nzÏÖÕ>?¼Ôc|ðv?²}\äWÜk3FGL J0301.8-7157@r ÿâ£ÏÀDߏÿ¼ä!À9©&Á½¥À;ìAVâdå¿ýÛZY<Ý+@ѾÎ\nì@ -à
q¿æþ¶"Ç¿ê¿çd…'*W¿é9ð¸Jšê¿ïþ×;ï"AGNbcu?ïýܜ¯#?2S÷…ñh?€ê‡É?[ý¶?*.ô˜ŠÈn?0Q'^''?ï¼ð1\T?|ÙË´7úÙ?M9&·;?Uï[F'e?~Rãjr}?yüUhÒ
Ò?ïS>յǜ?}–ªš7M?"Øg³\'?sËø•p?†WâÞý¼M?r]Cñý?ïÙNŠ.†?rÃ{–ðƒ?&&Y¹I{Ë?CÔ²ûüO?r§ˆ)ñ!?rYšjÕ).3FGL J0301.8-2721@k =ÀTïFÀN‹_ !¸À:ÃhÍJ¡À<îл?Í°¶h)@
`+¾ß@CA¿½ð'?ßóä²áX¿Õ¡ Á"–û¿çšS|:p¿ãºØ0AGNbcu?ïM–¦eY?'{`ôßë?~æã½®Ø'?Œ5¢Aº:?€9(w=Z?'ö›âÓÃ}?î ­Ë«?°úvžò–=?'·iêø?™W›®Ú³?¦CgKnOÒ?©#1àÎõ_?íW~p¦—d?œF	…À?£ï'$» Ò?"ë &Ãõ/?¦˜‡ÐÛhÞ?/žºñn?éÀtƒ‹?¸ð½Õ»ÔÙ?¶~GAï'?±€ ZQ¡?½|{µô
?¯½yYB¸3FGL J0302.0+5335@aµt!-wÀÎëÿÂîRÀ9±ôafLÀ;RN©±>Ò¿ÕáVՂ[˜@­Sk7¦@'€L–‡¿Ó^(²Ú:ý¿çl*³e{¿ê½·õ¾ø¿Ö—I³'_@AGNbcu?ï¦j'XŒ?…™Ä:Üí]?}5M"Ûl°?€ªIJC€v?o+=ÌðœM?vV®x)?íà_ýyÛ?³ÙT![{\?}£¨˜$aæ?¬4¼RpQ?®E™½#Ö?²À*ö?í¾Þ×ÁÒê?—Ìœ‹¸õ|?›* ?fÒ~¦JV?¦Ê=MÉy?'>™±vï?š©;ä?"ñàþ'n?F¥å7aï?J'7cÇxY?¤1Ù×d=?"ßx¥sš3FGL J0302.5-7915@r|>KZÀAýVÿÁßÀ9æêºô]À;¾˜Ã°ÄYÀÆã<û³ë@:Æ¥k_@R_žK/¿âß
e²ü¿è†BPÿÄ=¿Ùv?/Y¤¿ëæŠx
õõAGNfsrq?ïø'.qål?JÙÑrœ«?yóÏÖ@?ÁnÂ>?K辆µÏ?JQ9YiB?ïÅb•dv?yQ¾Øý?LeçåiSO?Uv¦"±?yÁøQËÞ?v2ޘÿK?ïÆ1Rm?‡²Áj'3?`_'½ïú?rz 5NŒK?"·
Aà:w?"N{ÿ«?ïäÞåµÒ?m[»¶H>Ýÿ#ÔãwU>ô}éÄdþJ?kè!ˆ_¼Ó?m	pN´Þ,3FGL J0303.0+3150@c"CŸý`éÀ79՟Ú%{À:1æÒ1œÀ;ª²²oSu?ét4'®ÃÍ@
š{'pÖ,@…¿rÇ¿Ú¹éï¿åsÍl¯Ö¿Ù¾Uà *‡¿ïÿÜBê}AGNbcu?ëŠf7[?ÀK¨öLÉ>?¥ñ6Ý)ߺ?°)Ç?¸¶i_°7a?¶Øõg¤è?ä$­5éøÍ?Ç2îÒQE?Êñ"àÊñ²?ÁÀ¯<ó²Å?Ä{·G+?ºJ$†2àÎ?èw¥R_Ӟ?°=Yé[
?À2qdþ$ ?§hŽ†Ó#ä?»Ýò£Ð?£íw¡›ÆI?äãH/	Í?¹ÓKHHêÌ?Á¨áøå?µÞÕ½ØpŠ?Êå6b¿å?²†œEØ'3FGL J0303.4-2407@jÔ5 ÝDÀN‹`òËÀ7qJ½"sæÀ:¥C'&Ò¿ÏÓXî@ÞõCc'?þ±Zá"Z¿Ø,ôˆ¿àÉÇ{C)¿Üs,aK¹¿Ým8<²béAGNBLL?ïó©'5N?Z/Ir}ˆ?lkrÙû}?ýKf0 ?X	˜iþ'f?Z
ºPüú?ïØ4‰[v:?u{\SœÎê?@Ö$Rpä[?Kà›3fr?qÊöÇöÇ&?s•¸Õ›—¥?í‹ï¶Žg¢?¢©už)*£?'$øNæ"?~¢= ÄÞ?±\¬'æ-?¡Õ"*??ïïû	û?`]áŸß>›'Ž'#A>¬¯ÃЇÚ?`dŠËÀ?`\Ž~°r˜3FGL J0303.6+4716@b ŸDÔEÀ#¶î#;nÀ8SJM++þÀ;N"šVWû?çÂ6oÂts@å-oÏƧ@D¦€1釿㞎ŸÚ?@¿ä¯àWæh¿äú"â?¿ããœl²°ÂAGNbll?ïÙo
˜Õ1?wã%òüå&?Gd°hVj?Gý'»±?p[䦊¤»?v~WêUü¼?ï[¤Bª˜?¢ñîÌ<ŸÈ?l)¡Ü²{y?u$¾a_(«?œOW<]š?¡>_?ªw
?î'46¤¼?Œ½\ljJÒ?‰bX÷êã?|TF{3F?šüÑL¯s	?…õL"7L?ï­.@ú£?'|ý›¡`³?7þÚ|??€•D"ùƒ?ƒû·ÑLH?'XZŽ"™â3FGL J0303.7-6211@qƒÄßÎ1QÀHZ$™ù;À9!ý¥²¬À;´Ñ¤¢â?絶"ï̵@ëxˆ§Ú@®ZÀr¿ä8ÚSÀhÞ¿çVbÔ¥M¿åD'â7†¿ê€?(ðö3AGNfsrq?ïÝJ]ã?nôÿ4Úè?RE«Úžs¤?Mãòî¤L·?i'Ì/ ³N?kaw¢ªÇµ?ïN/Ô«®?"Úˆ'›®"?dî—z·4?i†þZ~›?"œ2{Hj@?'`¼‰"É\?îî)'ç®?‰riLÞg?ˆ¸
P¦?xÉzû…†?•ÞÏ}â4P?ƒS¹F箜?îB[#ñ‡$?¡Ќ$£ú?}Do–§?sM¢~Q>?¨9E=ùšâ? 7=.Ëi‡3FGL J0304.3-2836@kõ¤€èȬÀNWþKZÀ:òº.d—YÀ;æÃ$º?ðíÇ¢@gËOKE?ù½AÑ6>¿ï»¹/7Å¿Ý㔏nm?톣Ùʝ¿ß…±">jAGNbll?ïßèH»ÞV?q˜Ôâ"H?RàtE®Pi?WQƒ»?f§}!J¿?om™ÝÐø?ïp22åˆõ? p¾\"?fµ'"n?x[ƒUtªh?Žq…â]¸?œSµøin?ì«ÉAÁ{?¦Æ&ò¾W?¦§g/ƒ?™ÖTKY?¯IÜb¸Á?žgj`%é©?îJTé'j!?³¸•—Y6>?U`šç?wÅ~Y`2?ª±øz"†®?³­jµË£3FGL J0304.9+6817@`Ù´ßݵ@!*ŸæºµÀ8±ÕORM«À;PgžtÊ­¿àiÐu›/@‰7jöC@Á`)áP¿é]£G©s¿ç5¬âC#
¿éÞ6%DÌÒ¿ãQj͘ AGNbcu?ﺵ"Ú½€?Îy®è?sÒÖ*+?wŒ¶ëÂ?m¦:y@,#?t‰|וß?í"rqið?¼Œj~öä?†ÛúùXG?'ÍÍ
@Œ?µm5…€?ºu‡Ú'?ì÷Zu±×J?¤½£LhyÏ?ž-"ø3L?'~ w~?°½àñ38Þ? 
1ð¦?ìöōõ²­?©¢7²†÷?€ž¦G/?6`ì$<?¶G?»'a±?¨øTqP/´3FGL J0305.2-1607@i
l <K
ÀL'BàO`À:Š:¶µ3SÀ;Æjd!èˆ?ç·Uðêc@
x¯¸k?û!Û­?ïºSzÍR¿éévÉ¿º6'äÌ¿»Téj¬
#AGNbcu?ïÊ_š¿[´?zdëI=sR?@zû*Fº? 4›m_¿|?z[0´e}?zE/ËV""?ïÀµn"+?$Éi¼/|?N÷uåHD?T½C͏?{ÆZIaÇ?–f2`q?î/b–ÇB?'´â¢DÊ*?ŠÃÀâtXK?{DmŽP2s?¡\öuÏ?‹ÔR3ˆs?î/½{@ˆŒ?¦Rnõ á?OdII(Æ?rçה'	?¬†—'zR'?¥¥öMDèi3FGL J0308.0+7442@`w¿Â"O@,o[Ao6À8ó¸ÒDÀ;Ý@ï´Xb@H² y@\z-m¡n?èh°n$ÿF?ã±i¸"A¿Ò:…ÚAvå¿ç[ooyŠ…¿ïÿñ­µcPSRPSR?\= ¼tØ?kK¦é›?ïq)`r?¬¬èmTUP?åö±è?«æ'Y-ǐ?_šZ£?|»Eÿ|Äè?î½VÏWÕ?­P(¦Ïy?£2'V7²t?¬ È«ª?©ÁÕÇ'>?›Ï¾¿Ã#?ëqÚ¾ÿ?©gd‹Þô¨?·­O$t?¥'£À¤	?w1ªÖX'ÿ?tb¬ɾ?ï~ÿ(ÿ­?¸œ_0ۈ?"§`U
€Å?	1ËU3FGL J0308.6+0408@eÜ:Ã.¾ÀF;à0VàÀ9¾Î?""ÆÀ;#†Ö?ÛÏÐÄsq@ðE®_ú@'‹ßǦG?ïðBÐ+ž¿ê,²€=¿Ì¦†iр¿â¢æ1ð
AGNrdg?ïâÊ$g²x?rtÚ¡UL?(Jw-]÷U?+Z!‰¤ùT?k±4%w§ö?rh⫎?ïoãždډ?[†E´Ý?cI›¹Ééž?fCžŠZ?4±xVãM?­‹æñŽ?î[øV@?"
'ù¾?†ø¢ü«#?uèSuôÞ?¡Qô»qF?Fº¡˜é?ë­*vY?³vG›Í‹C?p¾¤•†µ?t@¹ð Ó©?ÂÿV6ïc?³A¡þ^Å-3FGL J0309.0+1029@e%F?ÀCێÀ!ßÀ8kÖÛCˆÀ;-T®­ýÕ?öÝ7ì*‹@™»þHp?ÿã»(Š¸¿à.–PŽã³¿â]ÎUŸ*¿æžƒ8â¨4¿ä
(|Bh'AGNfsrq?ïð†úžYÏ?_'µiÛÈ?8Bò®?7€+¯zò?XκžØ?^Ö¨}¼?ïÈqøWöµ?xçëȹ*Ò?G‰T
…ƒ?PÂDG?xÕÙCãTe?vÌE,PÃè?î-NnO‹©?™¿¥çF˜?™ê㸓ˆ?)¥ÜÊ/à? £©*û›?ÁBéSªŒ?ïçÏæ×[?nØE¬÷"?? YàQc?0Põôà{?g³§"%?nYrb¡q3FGL J0309.5-0749@gš·?1n7ÀJWÿ›V2À:åsŒ¿—À;¬Æ8^_?Ϥ'౟ä@Lªhö‹?þöý?†RÀ¿Õ}¥kΞù¿âéC¡¦"?µá݈ºVÜ¿èœ)×È\AGNbll?îñÈE50–?­«©9¶ò}?U+ÀK)>?WZ(X_bP? :ªS­ß?­|%Ò·»e?ïdÜ6n)?e;H+&?h)z{j?lú&<B¯ô?_IâÚ̞?ŒújVâ?îÀfR?žñ&h?—ÐÒ»òwõ?ŽªzÙÜÿ+?£‹<æC?•'PmñÚ¹?í¥ -X'?©[o/pÒ?^+qE¿w?h¯=ÂÐî?²_:$n?©9RÝÈ3FGL J0309.9-6057@qa¦`ɊÀHyðßьOÀ8Ÿ' <¶À;¸éÀùZ?èªXðeÞ@׌yËs@_žŸ½Êü¿â!©¢?h¿çÚñA
¿ä;Ýòö}¿èb]{AGNfsrq?ïò
´¤CL?SçRr¾¿›?2Z÷EÁú¸?2-2]'ÙN?WSØæêú?R¹wFö?ïºÏ3p)?~]³ã%m?N0ª/?SP>ƒaìè?~ׅðEÖ/?{•j÷/ø?îþi_‹•:?†¬-—s"I?ƒ?`³ðF?wÚd^1?–"#µàª?€±8qxµç?ï—z'Y˜M?‰lNiš*´?=?[Ï¢ÿ?@›€üMT?‰7d‹!g½?‰.V»Ý3FGL J0310.4-5015@py'ß֔ÍÀKr<à[À:3maÚÀ;»€šŸS?ìêjûݗ±@õ;Øbç?üÈ>Ï¿éFчƒ?Ö[4®³\¿ÒÑe™žy¿Ö|뗬ô.AGNbcu?ïû†ô©Ùé?K§V–— F?#ž¤?]ÙyAji?=¿s/¯"‰?I÷%‡C"?ï¼²vAO'?€®6šrší?Oò§"]'\?TûÿJÈ?}¨oììŒÑ?~ë^t¤?îêeŒ¤?•e"Á@?Šåª'ŽØÈ?…_÷¡W?•IÊ*†ÿ?¼œp ?ï–"tè!?†/(ÓH&,?Zðä±â×?eu…W;b?‡L‰·6?"†ÌÂG¨I3FGL J0310.8+3814@bÝF€"À0ñà18‡À9›á·?œÎÀ;š­•Ïà~¿ø´Ô2œµ@cÏÞ$8@c x›r¿èÖÚJlh¿èBxŸñCò¿ÖŽ*ľz=¿ékë-ŠýŸAGNfsrq?ïýà0O{?6áú°çSó?¼'ò%tð?PPQRt?3‰ÚúÍÔ?4Uº3kó«?ïÅàŠ(¬?|ûV÷UGI?QÑÕ©NA?Wh «""À?x›¾VB?z•(EsŽ?ï9ú|Y?‰Jûyã?Ϻ‰›a§?y™vsŠ?""íÞIœ'?…¯ÙŸe?ïÝÐ:;žµ?kž'‰u>ã:½‡8Tñ>ùkÄ46»?qEƒm	Þ?k—0þá	3FGL J0312.7+0133@fP†þ÷ÂDÀFÁÿÑÀ9$5Ý1žÞÀ;×xø?ÒSDܺ@'èá'*@B¦@#¿áëŸè,œ¿ä
ÔÝp¿ãÁ&~¢zò¿ãÓgTmãAGNfsrq?ïà«Ä#Žü?p…ímÌ®?1ŠÉn¦Ë?/t¡Ç=?m"â¸ã.á?p…®b?ïÅ/¶—;?}W~$Ka?Gdü÷Á¾?RBÿÌ'	Õ?z‡H…¼*ö?zÿÝûËCß?îÛ
5Žy?Àpæ•?…k]­?xe¯ÀD+?™é
ÉJÚ[?†ót§m?ïß~·³Ó?p‰)êèSÈ?8Æç?!¨ùåN?pg´eÆ?pu½hž3FGL J0312.7+3613@ce`A‰7À2mêÀӚFÀ9ö"ö¥
kÀ;œ'«hÎö¿¡](þlR@Pà$ÃXÛ@E"…á׿ä'
Õ#»ú¿åàÆ£V˃¿âÑz­Ž!¿ãRt‡ï×AGNbll?ïÆéÙ-:?ˆÅF3"ì?AO\|`g?Då"t¡Íw?zaƒÝ`K?‡Š4WŠ?ïžÑэñ?‡N«µWvó?aÎb§h?d!"Ÿb¨m?"ráÜ@¸?…8°'{?îü€\ÂU¼?ŠÌ¼áÆ=?—¨6Ê\?n:œL2tÆ?—¤ L¨ãi?…¼VK'ç?îÚ_ÔÊހ?Šž'U…?TÞýŠ`ž"?QÛ*-L?¡³
Æÿ
?Š5ð"(†-3FGL J0314.3-5103@p…B 6mÀJýJ 7BŒÀ9˜0P)ãÿÀ;ÝÕC"Ó‡?Û«Qß¾
@oŒhC5@3üu¼¿æô ¦ò%U¿ãžlO'ì¿æKr7#¿Ù©©1£LAGNbll?ï‹	¼ir'?ŒO7¸?u'"øDeÆ?xΨ]fžé?'tiBÝ?…ÛíÀB¥	?ïnýb6UI?™U>­gz?fùa¤‹zQ?vO<ù˜$?Ž'O	GÏ6?–)éhjÀŒ?î"¯Úìć?–ŠÛëµÍ?"†1°Cu?ƒƒE\ÁL?£'ù8[•È?·ºRðÊå?î&3*4 ?¢:ÆS¥L'?|ô-˜]Æ?v«LÖ¾4?©þLwJ? ñî@9 Ä3FGL J0315.5-1026@h7¹ÀëíúÀJ=Ÿ¿™À:@¬˜yßÀ;¸­7Ü`À«Ðo¼@ÔÓêÎ?"@GÑ?Î!6¿æfݲMD¬¿æ™¡Ž|ýN¿×"U0¤¿ê™ñùWlAGNfsrq?ïý$	¹Ë?;9˜¤øÒ?[ôPâc?º"½¸ñ—?4Ô3©méÝ?:YÀïÈѕ?ïЋM¿'o?uÌÎóa¨?BÒ¾'ë7¥?Lûè>cU?u`[náž?t
wªtXL?ï1
Ÿ4c…?ˆ_·6O?~µdV•ä?uuؤÇÒ?'0óéù?"µwVf?ïï&¤'\\?bÔÔÂÈáà>»RÀ…iO§>Ò¯w"ü©ð?`Õñ€'÷h?bÒÕöÐë3FGL J0316.1+0904@eƒ  ôØÀCÌ¥ 8LÀ8aCRe'¢À:õÍêÙþ?áØZx2
@°¡€mΐ?þ©; jM?ßÄèÅÚGè¿âÖ¶ÓÕÞ¿ÜR­Ÿ¾`¿×ïNBßAGNbll?ï˜}R4²c?'ê¶FbsÕ?(é0IÀT?/cçf?‰}±¬gO?'ÖñP~?ïœý~×?"ªñr÷4å?W" €»$?_RM5ÚtU?…Ð~ú"O?'íÁçÏ›?í'Y€?¤Þ΂ÐД?Ï …'f?…†DÝôs?³L«?ï"ý?¢ñ™i}š‰?êuãê"‹?±>KðföQ?d¡À~2?iô¾Æ|?ÅÕéW"Ù?±DøÖ
µâ3FGL J0316.1-2611@ku‹y¢ƒÀLá@&`½À9™šMÀÀ;Ší~óûæ?¿^&"¸@'k£<"?ýµu_Óz;¿æ4©: >¿ÔS"™Tq¿¿ÓLw¿vš^¿æüv.õ$ÉAGNbll?ïè¯LwÐ?f‡nQ4?D'לýÇÖ?Dêµo*s?b,/ÌH¿|?c_RxtR€?\ 6?ˆW´4¼?_áý<­ÝC?eÃèáFÂ??‡ÛiP\¿¢?…ˆO*	6Œ?îí¸–-7C?ÞIyY¼Ð?‡$ÇêQE«?zÍHÔMt?–¶‰E0tÐ?†¯^€÷?î-=¿®Í?›ÜÉt|í?aÊÀÎJR	?búŸÍûЮ?¬x`n?›¼ð\˜63FGL J0316.2-6436@q˜Œ€AÀG` SÇþÀ9™m~ˆœÀ;Ƨ‰Fe?¿àáÕ#[W@)f],+@»ˆß¸ö¿æ¼ö‹ÝÕ¿äèåËæ¿Ømÿ!ˆ»Ñ¿Þ÷YñÁsAGNbll?ïæ`z¸V?n©±Mï?*ŸÒX`?)õ3KL·(?gþ5‰J""?mf[Àú¨Ê?ïªëT¤é ?'4ôåêò?RÏ ¡H?YâhU?'ë6Óƒ}?€×õÆ0Ú»?ï)ìJ?î÷?ˆ"2-I¼=?{-ªüŽ ?lN¯&'e?"÷4ýv?"ß ô:׫?ïdŒÎs;‹?…œíÖ¢—?'C›Yƒ5?4rbšÎ?"?à(aۓ?"ú0Ÿî3FGL J0316.6+4119@bÅ}q?À+xÃß¾AÀ9š÷È3áÀ;1‡ëlm¿þ?0Õ4û4@
Acôq+'?þlËð¦¿æb;qE< ?ïéå}Ya¿âÂÝÌ4² ¿äTæ–nä1AGNrdg?íÿQ[0?¹¯Þ˜Ÿí¾?v±NªYõ?yé¸9g?µ Ûχ6?¸Ócä½Ò?ïnàÚÐ?›;;3-?pTؚՉ?€®Ë»Eí?Œx],á(?–Pü«~Á?ì¶}b»óM?¢ìŽ‹*?œ	䬰³n?‰C¦"sƒ§?³I›¾ô8¹?ŸgÃ*L>?î'#öò?±c©gfpò?‡:ƒšJAj?£`,Ž8õ?¢¹>O
?¬šGH*¹3FGL J0318.7+2134@dZ{ 1ίÀ=¦B 6mÀ9CYLVÀ;FüÎX%¿ò%¶Ëƒ¡‹@ZaðàÓ??ýeŒ¿@)¿È†ÙI»h¿âÒÔ
³È¿ÚêYùN=®¿Å­åMn•+AGNbcu?ïüÖ+y˜?;dä/©rÜ>ø±ÂÄ>÷IÄðÓ!?7È/d?:Ð`Âì¦	?ïÎi-"b?uÈw±Ú<a?Izö›¹©ß?RՀ‰	8?uœ
›WÅ?sX¯¸nÞ×?ï@ŠDK?""CaAs°?}öe܅å?tBj]jô?q& U$?€`u/ÏMJ?ïÖ
H€p?j:Ç_‰>ÂÉêݱ&é>Ú'0vÆ?tø''l>,?jšn1Š|23FGL J0319.8+4130@bґ"DžÀ*ƒ þ}IÀ6VdöúÀÀ:C,x.?úw°:ÅÏ@»ªõâoÌ?ÿŠ\º³¿Þza+OJ¿â%^>#Ò¿áXïYXz¯¿äĶ köAGNRDG?ŠùÇ?­¡C Â¿?Pðò؀?V˜ Ý½±›?§,bý?­vÛt{2'?ï¯äh•5î?‡Á«¢à?WLyw¢G?^¤èdžÏK?V«ÐP(?…l¦Õî•V?è:\1]W?²OûT‰ÌÎ?¤-»Z…f?—ÍO€5&Ö?ÉóC˲éN?°£ÝÊŽ‰?î'v?ûS®?¦)‡*)?IOD¶Î-×?]L/¶š–?¦ƒ^íoŒh?¥õ·ç3FGL J0319.8+1847@d¢ß?–À?¬",2À9a6€Å=À;+£»[‹A¿ëq†œ€˜†@W¨ï¢æ?ù&:è¸?î¿^·ñH'?ÐG¢Ó¡t§¿Ñã%•L:¿È›ÀCì-AGNbll?ïùt07Û?P+Èò,?×%š¼šA?
¾ÇÔ<º?Hq͙tÌÙ?Oós°¶©_?ïȐ{Òÿì?yÓ|ÁQ?Mø@3[DF?XÐÔý³Ð?wøº¡Ì?uÕ"¥<®±?îŽ
òsD¢?˜1QÙ¥?‰ói®?"o«UxÏ­? ¢^1Jn?•^x
"?û§ÐW?'GÊÓ?
WUª1`?V´Í[œ?ˆiÀì@?úPܺuH3FGL J0322.0+2335@dCsÿ¬*À;—ý_;ϺÀ9P»Ú6BÀ;F>{?æ°5­Úñ@$Š
ÛPH?ÿ"«€÷·1¿àtŽì'Â"¿àUšéоŸ¿ßçÃô*¿× cڒUAGNbll?ï­I%ù҉?šªˆ€€?Tr§¼Å€?OG?øüd?'aŸ3Å.?}fÚ%§š…?ï Ð²Ò?†jÍ©zõö?]
Ï&´œ?`†èØ"ôi?"*€öôï?"™A\,¥Ê?íØ¡7Lh±?š=ïžN÷î?–l5•äOˆ?ˆˆY'ß?§?ÑÀGM"?"}?ë½9?í©îíÿRã?˜Ž7)ËÁ?Uû¾rh?XÿmWÎ?²ZP¡ŸN?—ؽ‹ž`3FGL J0323.6-0109@fþßÞøH|ÀFœäÿÉy[À9tJLTliÀ;i'Q¦»Á¿Á7ð㓞ê@
¼¤ªnÓó?ý¡¾ Œ'u¿äv%7êI'¿Ú'e»4Ž¿ÑíÖ/ª›'¿ÐñèŠÃgôAGNbll?ö^*š?¢E™Äre?U©ûÕ1¡Q?T¨Š&ì")?£Æà»sÉd?¡ÁQ:Dm?ï¡F`ùñX?',òÃ?Su¹9W=?YÚ·NVÕ?…N9
\
?€"ºêÈ"?íµ¼Ú%×?˜=ÿqÌ*?"€È<ñÍ?ƒÎ'×ïIÍ?ªcÎ?Z•¬?˜†=óÕ^>?íß
³*¬?œÌ´y¯c?DÆ6à?JÙßZ?°ßlÚò<Ø?œÅ³ž`À×3FGL J0325.2+3410@czªŸ{ZêÀ2±Þ_œGÊÀ8ª_!ΆáÀ;r‰EŽŠ?öÖÒµ'@º³PÏÑ9@¤Íˆ´o¿åÖ2¼•Çþ¿ëÕf7I¿ëp§
ׅŸ¿å)y<¤AGNnlsy1?ïøEÖD‰·?H¤É£cœ³?>甂:èý?;Ìn¥–?>é¹Yw\²?A@üȱ9?ïs»ëíŽ{?–gSm(z?mˆ–Gåž?xºÂ=øªn?‹Ëâß
gÛ?"®tË̞É?îoãóÁ?–´ýÿžó?"2á#^?ÚÄ^Pì?Ð¾»d•?çè§LÃF?î~t¢ –?¢"3DRX
?€8%óâÁ? ¾QxN?¤
¬Y®€?¢DÊtJæ03FGL J0325.2-5634@pí ßÞøHÀHîà_PÈÀ9ø¦wÎm·À;øñ¼p^7¿ó¼lzQªÃ@í«B¹c@¹´ß›0ž¿ãu'ªMW2¿ÝÊÉTÊÚ¿åxþ(º^`¿àX ŽAGNbll?íìÃ;£IÅ?´IT|ÉÅ??x7ôL;.?•×l쑠›?®,ͼCýß?³5ŽdÙx?ï'éñNÇ?"|æ×¹ËÅ?[)}uÅ^?i™e܃?‹àSúi•Ý?'e_ª=çÆ?íz{JEØy?í$[àp?š]škRØ?‰O/¡¨Íü?«)~%ùS?—<ñËÞv?ï>°3Ã6?'d¨T\=?E»Œ"v?R›iȼ«?—|!˜¦¸S?'/̼²J3FGL J0325.5+2223@dub¯È°À<I¥ÒÀ8hpeÓÀ;Rs×Ûõ?õWéÞ«qˆ@BFBÚp#@¡êöÙe·¿ä¯ñuVKð¿é1-o#ú0¿èæ¨ãZû¿ïÿ?"éøñAGNfsrq?ï÷ ¿« ?I¿ÒùéŒU?8	ô*¾ú?;b<×Ò•?Ex@>Å?C´·W1´?ïqN¨	–š?'<hÙá"?jªZ´Ñ£%?ròT¹"h?¿Peð€?Ãð譈?îPyÅic?˜Ç$M'k? Dš[сA?'Q2ˆ#½»?•g©Ï¯Ñ?Š[ý ¤ù‹?î EÜUd? FÓÚ
M?€͊ü‡Œ?'¦´%]?¡úî܋‡É?žäjtÏ¥ç3FGL J0325.6-1648@iÀÊ`ÀJy¢@1HwÀ8þ­-]À;.InÞÚì¿Ý4gX\@ØOØŽZ?üì¿[u?¼â¯ã ܿޙ`æÂ
οÚìýf?¿É÷7ô&óAGNbll?ïîJ{•."?dkóÇÊÐ?%ô{Iø6~?)ªÓ['W?`V<¶2[5?c³%*æÅ¡?ïÌ­pžY?w-dE¨Ï?FïÌl:CT?OÞþkmcÕ?vËN#l
û?uˆÕ…ߌ?îÑGÜ?'D}²¿?†Ô0ï+[?~g¬çÎiÜ?šm¶ºVØ?Œh¢€ûþ?î˜èí>'?"Ôåiƒ	ã?RIÈ«Ík?(i£qcu?¦pˆLGǝ?"Ô3T´F"3FGL J0326.0-1842@iý^ß)ÀJÉ?Àà0À:P3:~À;ê'Ô©:!?̐õ_ß'@"KtG¥†@¤ìԍ¿ç­üÉÙl1¿ë¨ËÓJß?Îq€Ö()¿å)Rü{;AGNbcu?ïÍuɕ¤í?}3jg+3K?#mµÁx?…ðƒòC?x؍~V…Ú?}	öLÿ²?ï£ÝMö)¼?…ÚìGøË?V´Ÿðâ©d?`'«¦8¤–?"2"Y;À?ƒ™ë ³?î{ë]®*º?ßêԀ²?‡ôÞÏï#?t+"VÜI]?¢ÌíiX?ŒäØHº?ïÙvkÞ|?œÃ5¢›ïÃ?5 ÷ʞ‡è?Læ(%®ç¤?ŸŽMSY¶Z?œ¸´9²O3FGL J0326.2+0225@f—ðŸ¥LUÀE7´_î}!À9^9£¼¡À;sK@p2˜¿Â2õö¼µ@Pß:šˆ?ÿøaՈ]¿å>êUÁ¿ß‹ß¼éá¿Ù¨ÀdDß¿áà¼:OÔAGNbll?ïî¼BÀâ?XèÜ´ú?.d!Á¶'±?({³…[Ã?^º÷œGgn?W‡ãµ–Ý?ï¢OÊûmo?€çà#¶?U2>"8®?W±±ßÝ¢?"ÅÅn'üä?~UÍQ1?ï0¨6.>S?"!;ïÃúÊ?&Våÿ?s¹—"îÞ?'Wªr€?~2r®M¯…?î…ý»ïáT?ã(х|?H3óÿnn,?It¤v•áÜ?§?Tq1?+ÈnB3FGL J0331.3-6155@qO{`(^ÄÀG)´Ÿ¯]PÀ9¢ó_2•À;Ãþ+êi–?ßʆ˜ØJý@JêßÝK@œÁ€hp,¿Ûh€{¿áýý–æü¿ÙS	÷>0¿çè0ˤٔAGNbcu?ïÙÝÇZ86?€ÿI ãeè?O5Iå'S½?ZtEѪÍ?nTæ,c42?|}$¦Ê?ï4]Wiؔ?'"¥á¶~ü?m¤fZÿc'?mŒ½e֖ˆ?•¿ÈGe
?]cu€?ï
FdµŒ­?‰æEYðÛ?…A?dÔ.©?|¢V$µà?"¶"¶äS?A"áãkR?î'»Ó³ÿç?™K
"óE«?užØ+Ùäý?pނn×'ì?ªÐg¿DÄü?˜5å°ó3FGL J0332.0+6308@a~] Y§;@Ø4¤À9Aq
.W+À;E}ö¥ä+?ډWw`3Ç@
~ºÆ@¥àŸgŽÚ¿ä@Ë·€¿âbƒp'o¿çü5ïêÍØ¿áx¸É	É­AGNbcu?ïs•ëQ?Š.ôuâà&?w™Ür÷½x?vÜJ–¦³]?‡M—½
*?†¥õ?í3Ù3Ÿ·?³á‰õ ª›?zÑ]"QXY?zŽÛn?´´ •ì¹?³3Q$$¹?î2Žt¼?˜@ÑzÀÕW?•|L,]'?ˆaûc'h ?¤š˜ø…ƒ?' ½ßå?íoDmì²?˜šAâEÓ?UŠ×-6U?{ßíh>È×?²]ªó›?˜[¥7ü­3FGL J0333.4+7853@`Pz WŽ\@2{Ä¿¸TÀ9Ç~è=k›À;Ìëô°@¥¿à— ïèõf@%Ê>ýí@"Äÿ£ä¡¿Û•Dí'6›¿èñ%Ž¿Ôº˜ñí²d¿â_†«ßAGNbcu?ïÓD×úõ?yÁNl¹¯?:i¯p$3D?:4äñÏ>?t·VAü?yPç¸"¾?dÕÿ?'ú[œ
å?ohûŠÈý?p"%À͝ù?"?èݍµ?½R³¬ñ"?îÜD+ÿS-?¿öýÞ,Â?…¨t&?x?v™Ãw»H?™î¦FzŠ?‰eƳc$Š?ï?¸æGš	?‹‰—ïÕZ¸?E^ˆ™õ ?J{R¢Åúµ?—`pBÇïs?‹çÆKÐÌ3FGL J0333.4+4003@c3›Ÿ˜·À)óš?±Æ·À:ã'ñ·À;"b£cF÷?î…pƒ[û»@q¡Šÿ¢ã@æ¿ßÿY'?ïý°´,0Ï¿Ç$ۛ`‡ï¿çþÏ$¯¦¿ïÿ	ø&mAGNbcu?Üi‹î˜LÇ?ÍõÆ»vL:?àáË·RÝ?΄®-[?-ߐØ?¡oî'Þž
?ÅIRAÊ?đ'ש2?å¿É©"W?ÈԜ¬øV?Æ;ê‡Ú?ÀPÄªW¡?ái²]+?¶uÞ_Aõ¢?Óð±Äg I?³Ù|zŒ?äõ­½+?«tœ‹t%?ôvՖ…?»ûé13F?è1~ª{¡—?ÃVÈiø3?·†wÆC?±qgs¸šŸ3FGL J0333.6+2916@dªKÀ5…šr¦çÀ8ÉðeXImÀ;=¨;i?ï-@ÓÃ6 #?ý¶É™"{¿ÏgÆ°_¿Ú¦¸f
{¿ÕNÇ,ò|¿Ú‹Ù"׬‹AGNbll?ï#oÿ?‰ ="è?xŸ˜Jú?ÔKp#?ΰ,y~c?€DËNÙ*?)ÓÀ²?¦ø,&ál?…¥
Ÿù>?ˆÍe'#ø? |YñU¶™?¢Ëtò' ?ì¼úmò‰?¡3éŽcçÌ?¥3,Ÿtp?•#`ÝÄâ?¯&±bþ?–¯:Ãô…?çςµ«?®Ü´iJqè?"›š²v"?–H°Ô¯?Î.Ó!P?®tރ¬˜Ï3FGL J0333.9+6538@aUDupÅ@p4 ½À9SFS¡hÀ;YÜ&Ü㛿ë…hßÜ@•ÒóW{?ÿ-! a¿ágZ™t
¿ã;©MZ•'¿ãEMVlj¯¿Ã3{}¸AGNbll?î&CЎ¥?©òv˜§e}?j¸s1­XD?e¬óÿmðc?«ðG_Ü@*?©_òX¸9®?ígû{£«É?¼q·"?u)«G'Ò?}[ð÷¾Î?³m‰q.(œ?»@.ómêÜ?í`ëL­?¢oe–á?|¨±ü?‹N~Qð8?°ò;nR?ß,¸´.?ï$Ã.‹?"ŽÂ†ªt·?-t͵s¨?8ó»j¢?žà}þÓ(u?"J–€"3FGL J0334.2+3915@cG_ét£À+Æ 
aƒÀ:3æ/tbÀ; Öwpyæ¿ñ[µ
8h&@	'C¼˜L=@èØÞ\—¿ëž"('D¿áî‰~ª'¿Ñ§ˆUà˜¿â®+VÅßsAGNrdg?ïör­iÓå?dÎå?&_‹ªà›?6é:N.î@?PN³ºBÚt?c[_ñç`?î¢þ °ó?³A‰CF÷*?†ÞT]]"q?š¸žçÓ0? €Ý¨l?«ƒ®üHŒm?îƾ{Ö?ŠSŸ¹aâ"?‡ö"ÒÚ%?u VÔ۞?›,ôÇ}Qœ?…EÏ*Rfù?í—Âe˜?ªøe¦÷?S¸_w¦§?YrñY·²T?·œ`s.ô¢?ªŽ¾ì@3FGL J0334.3-4008@n˜ºà;>šÀK{Ÿ³À7ã$Õ¢^dÀ;ÁÀ)P[?÷	ÿºùf@
PIC•×@΁,æ=¿Ü¤SÃႿãoç‰ðõ¿ãT!šsx¿ä2Ó:éϬAGNbll?ïóü#_?Y4Œ­?.'Œ39ÿ™?1jÖO$Åæ?T7–2Ú²?XA¢Ó¥·?ïÌo³H`?yçûØ,Ё?H/Àÿ›Pì?RdeÖÀ|C?vÂ.;܊º?w[€¥éÃ?î—òü"?"ëªÉd+?.°Ÿ\'?‡®ˆ~H4,?œÓ¡
¢?ŽCóyI?ï…à€Êà?'uz¤q)?3Bns³h¥?AQ)Û·?Ž!ôl/¬O?'}œ—ñsù3FGL J0334.3-3726@n¶â—ÀK.Æ 
aƒÀ83A!…À;é/"Ê?òd>0<]Ô@@WŸÏÍ?ÿD@v½¢¿Ù?…¨Ö'¿ÞÐY©êt¨¿à
ƒsVS¿áÍróéAGNbll?ïõì)	B?REîØ^V?#N{ƝÕä?#y•¸ÓgÌ?Q½ÝMÀ­?Qt¦ú°Ä?ïœs•àÑ?†`Àâ'7?[8K¾?aG˛	¦?…˜!³~h¼?ƒèL_Û;?î>-RFB?˜×éPU‰?'–³kGIñ?‡‹»Y¦)?¢ÑÑ%úÖÑ?"¯œf·b?ì^5{€2?¦¦§Ò}?vl±*{?v±1.îT?»§‹,ëÆ?¦O ÓÝÀ3FGL J0335.3-4459@o–``þG™ÀJs^ŸÈ‡ÄÀ9Èi*–¬À;ŸÈå·^¿ÿ€˜N?þô@ÅC–'¹?ýL ?µ?DkYÀ;¿ä3JJZ¿Û¹69y¿ÁíõçMWAGNbll?ïðÁ¨Æ2??l"0Hæ+™?j…@?#GøÿoéV?\¼wË«kÍ?kæóNÿ?ïÎñÂхq?w÷—u?E8¨ñ;Î&?Q×á¢sŒk?uà	y͕?uYÑ-(½?îý˜ºï'?‰`AÜ]E½?'æ 
–?p'ž­)Ï?—FõRÈT?…±«‰¤ÛF?ï¬vZ`ÿ?:(—S›>ÑQó@‰>å²?ïåÁ?"à?)X=O?9:ÝðÅn3FGL J0336.5+3210@cã@¢‡À2ß?@‡¯ŒÀ8¥ÎÆ¢aÀ;£êUt?ð"éŒùM@†GqD@ÿ•!¿éÅÉjý
¿é—£‰â¿ï50ZÞj¿ïöZNÍdðAGNfsrq?ïóf],Ït?_Â#bíkÍ?Oó¦öŠi&?ZV‹›?BräV7À½?Hù=ëU,?íÍWf¥¨?´A=VՅÅ?š¡oz'?¤üw‰«+?¥ÙÖáØdä?ªMڈÇò?í{D·dj? ½%0Z¥?¥^Ð0/ãÖ?•¿K"ø:J?¢ìäY‰|?–eVeei?æ%ÙïÔ>²?¹(6©¥?¿pJ›Á<?´¿ªq0?Ç°ròÎg,?µÍ攉]3FGL J0336.9-3622@mÉõÀv}5ÀJó²ŸúÜ«À:XSy#ØLÀ;ç@Çplz?ãoú¯@Á@«"ªO@}¾€ƒÈø¿ã¡EßL$¿äM՝Î)¿í2išV
¬¿ïÿ¬vÒ*–AGNfsrq?î''<I?©V«Tiš¸?–M¡O0Ý?œ>79öpP?—ÛÀ.ÉF?¡›
µ[f?ánŽP9?ÉÚãÝÅô/?ÐÞEX8ju?ūƺÿÕ?Ê»…ê.?¿@ &¹?ëªW˜Ž?¤ŸÙ…Aï%?²€÷fL"½?š¼_A¥ù?´©µÜï
^?ìy¨»y?ÙZ£ÄÁ?»¹e؉ï°?Û¥5º&?Á-"eI6?ÆMœ´H?³Q>'<p)3FGL J0336.9-1304@i+eà.©aÀHr¶?¯À9÷×fƒÂ˜À;Ͳ¿-?¾ÔT1Qÿ@
I—è¥#@\ 2e¿çœX¸uIP¿è
LTþp¿ì,í4‡'Q¿Û Kb\ŸAGNfsrq?ïQ¬æÅ?¢cýéŸ
Ý?n\"~úP{?n•Py‰¸?'þì"H[?¡Ño#k?ï0R³¢Ð?¢
øHñ?qsú:ð@»?"bÉïü.?•˜ªýõÒ?œ÷Â^ž`ž?íi ÛH™_?OþQ]?ä?—ŸlÇ8°›?"ÕÀ½×4,?­–;çÚÍ?—ûò#Ԙ»?ìõ¼9÷'?¨±MdUH?‡äþ'?^	­ôH"?µU~r%AF?§e
­®e3FGL J0338.1-2443@k\_x5œÀJNVßà¥ÈÀ:Ç×-xßÀ;Çå–È.?qê™*üµ@µ
a½_G?ô"=!±í?çÚ«»ÁGð?îàÃdCK"?Þ²~àä9"¿¼y¤Ëj¼AGNbll?ïÉnÂH#'?‰U•ÍD6Ä?0õåׇ}J?9ØzTú¼ò?z9@~uÀ?‰G»ðÀã!?ﶖ…r]Y?'kf£
´?M12-:§?T"V¦1m?€‡K€˜%ó?'ê®°óR?íᅇê©Ð?›ÛûeñÚü? n¬dãþ?–¨7(Ùr¶?¡xûrM?'}i)ßÔ?ï"w{•¢Ù?'áE«y?;ì8è×?Vl'~ã×?Š¿Z'ZÍ?'
aä0ƒ3FGL J0338.5+1303@e±ú€Ïž8À@uç_ö	ÝÀ9R&"©x4À;+_ùdÛL?ãyc)?@M<yØÞÿ?û'Àä6K?ÿ
¿ÀpÎ^È7g¿×ë´Š¥z¿Ü
{ÐA1µAGNbcu?ïçIþœÖ+?h}";¶)?CULÙ@ñ?C`¢¡)?cà®,é…Ô?fòß.x$?ï{q·ç'ø?r§;?c©R"Ü?gâOæ±Ä?Œ_g±vŠÚ?HC¨º˜?îž[û'°6?'Ÿu"§Kþ?Œã'ÑË),?ËVc˯?Â·¤Äd¾?ŒûÊæ(°Ÿ?êêMï"®?®á¬:žf?'ò'>?Å2¯ø?Ã'©XY£v?­ê #x3FGL J0339.2-1738@j\¿ôw6ÀI"l?Ä;.À9µè«î0À;Âóá?âEz°AÉ@§¤d"ê;?þÙeÿä&[¿³ó€çWMÖ¿åù25Ý1Ÿ¿ÑÞh_S¼Y¿áɱD00ŸAGNbcu?ïé-õúúu?cW#RëL?0
f4qÁ?-"'h¶ûâ?dнD~ûw?bŠ1—æ'?Z´"?Š²¿?^û[
þ	?coèÔn¤·?Š~}ñÝü?ˆ'ªîŠaÌ?器¾Ä<?†êWN4"?ƒð AÉ?tS¤Oڋ"?•òèXôŠ?X*ʇl?í!ø¯…?ŸÃ¶îT"…?dzÀzG?i«Ï©áz?¶Li[b 	?ŸVð`"c3FGL J0339.5-0146@g€À
¡©ÀE9…¿ÈŒÀ7êûgPÀ;Ao¸õs?ø
ÃÁ
w@1sHL@«,Tò œ¿âBü÷Àt¿æ=ä²F¹£¿æË°ŒÇ›'¿îB"¼díAGNfsrq?ïÇkóoÄ?€`|pwªŒ?q?Œ¢3£?‡Nå\?faw§Ôo?asðûYm‰?ミè€`?}mwÐ8Žf?L6Z]	º?U.ÏoDpë?}0À}D®q?zʦ
øí?íã0†·"?›OÊfuM'?¥	NÅgÏ?"ø»L©?™‡Q³=Ý?IÿBݼ¾?ï¾ù÷
?†iMÓìWø?@®¸*¡
?XÉ£‰£1?~Üÿ%»?†Öy·]Ï3FGL J0340.3+4130@c9 _ñØÀ&;¹ÿkÀ8‡"õÎNÀ;YnÉw-@shÁ_†@qÁ:Gz?úAÔ£ÿÏ¿Ð$ð¿ßî¿Ïéx¬0—o¿â"‰ü²\x¿ê;õ2,ßPSRPSR?µž5#Kí?¶[÷K?êÀŒ+ÌT?ÂÀsælˆ?´åýQ~Qo?·¿{*4²r?–cÎâ´ÙÂ?±=ËRPWñ?é·¯
SÁ¦?Ã9¼sScê?ÆTÉîZ^1?Á]´(þB¯?Èî´ÒÁÒ»?³Ç´Ÿò—?ãÒn@P'N?¸Óv÷m?Çǒ+ûä?­*/in×ü?±'ÃX ý
? Bïíïz?ëùÒÊÒ?°1Esu8ž?¶-nTd?¨I ߌ–3FGL J0340.5-2119@j¹ fèlÀI—Ï¿ÆT
À9¨¹t*tHÀ;ƺ_ÿ¿Ó"(h@!͌Fµ@½j?¹ÔM¿æîNm)Þ¿Ø22ä{7¿ç§›ãõi¿çuê	k)AGNbll?ïãYzó~§?h ÖõՐ`?U«¾Ú˜=R?R±#Aç¡?aÐ¥Ÿ58ø?dÁ¯¶Ô$œ?ï¨PS4¾Ë?'¸¥HkA¨?T¨"³Å?Yl*å?ƒVØÑl·? ªâ&ð?îìò6[N?R07A?þ#û¸ ?'#ÜÚ±?"ÖºÖº?'boªœÇ?ï23ì1"9?tÔ¹ @4?b:Ö]§F9?hüHúDŸu?—r'®?Ž:I#3÷"3FGL J0342.2+3857@cu¨ÙºÀ)¡ÃA2Ð7À9c2:å¯À;sƒY¼3ø¿í$GÎÜؚ@8rP)Ž@ôR?gôÜ¿äSõCŸ£/¿é%©K­¿ß6Á¡å1¿á	pe)
ÌAGNfsrq?ïó>/={?[@wI"H%?¤›§cÛM?
¦'ù=h³?X†|òIëŠ?Z¾3
3ɝ?ïÆI>ü~j?~p'»‹›?Pͱäbá)?U'pÉkeB?x§ô¨ƒ?{xà<=?ïrûdÆ?Šøìõÿ"?wúBËé(?g'†¤ýø?—³ìn­?ˆöDzGÏ?ïÛC\_EÄ?hÛRÎñô>âúø+>ðg©Ssò-?rULD`ß?hÓ‰0VÇ3FGL J0342.6-3006@l|¡A(¿ÀJCr_˜ìËÀ:Ûk3TÁ"À<?'æFñ¿æmŸÐÀLa@ދÞðæ²?ý‡_úfŽ?ïÿd"$©>¿ç¡jé?¥d'qya¿ãÈï˲ùðAGNbcu?ïìÄ&"ä?hÊ	T«?P«4¼?*á*
¦à?bQYg™zÉ?hK—b†%w?ï¬<rRè‰?"#ëpMZÍ?R
}`E7?XÓ_°I1Ë?'°¡»™Õ?'µu>zƒÑ?î¯æÎ?Œíù;Sãþ?‰¥£×/ʲ?z©NÄ%[Š?J1RÎX)?‡ö+·¿-?ïä:Zy?•·\"Þ?%N݋7Ây?3ÛÔ±5Ð?œ¸Û^A`?•¯Ûòx'3FGL J0343.2-2534@k"$?åÉÀIÓ½ÿªo«À9dïS	'À;Áozân?õIu"¼gÐ@ÝŽ<_@z®YÒY¿à«îz
vë¿æ™,¡É"Ý¿î\+~LÐØ¿ï夦Î;AGNfsrq?ïàþ8[æ?rýç5ÝU?XÑØ[]Å?`˜ä
*¢?b˜Û£¸kÆ?ié.ô6ç¾?ï³0Ã?µI?ŒaïÀ]ë?S%í)Ûä¸?[
«Àƒk?€ÏŠ×18?ËÔ¼ˆ?ìܯâ;'Ü?¥9­Q»P?­%ß<ìÄ?4^HA<É?¥(Ûý•{?›˜qÞþ? úM?Žcu¨0ëœ?k'ä*{H?s–Ýù36ù?"Ks&vÍÒ?Š½R\PoÐ3FGL J0343.3-6443@qsb¯È°ÀEԛ æÀ9fÖ 2¥oÀ;´UhaQ¿ÖYÛ¬AD¡@ÌÝÚçÐ@;}ßÔ¼Z¿Î² yL¿æh»j—¿Ül3,۳οåÿ3¶AGNbcu?ïïfO½Š?`ÅôÆA'?%ú­²x,?$ÄH_¼Õ?^t‰ª5ç€?`¦ÞW¨õ?ï¢î)Žx^?"5B+¯˜?Q	–ÓXJù?TŸv¤Ÿv˜?…#BÁöß'?ƒHZWù?ï žÃ€ó?‰ÚÇ8ŸÈ?'ƒ­¾%Ò?vÅ{si€?"šH|ø»?"ù²7`ó3?ïFêâÝ^T?âhÙ¥?5p¤ÿ-Õ7?5Xl•€??–ÌáW~?Œæ,7
ª
3FGL J0343.3+3622@c°ƒÀ~à±À-fLÿyÀ9Õáƒ=6ÂÀ;x?ǖ,'ÀXî$`\Œ@ßE	¬§@i0`¿çWœ=Q³ì¿çޔiÂ7¿áÌøàÀ¹]¿ÝyHª­óAGNbcu?ï,»×˨…?ž‰rãm?dm¡Þ6˜?q	¬U?úÍ?—ÚÐÊÄC?$;	ú]³?g¹"?"'éãm¥?ao
qT†›?vÞ&ÝL(?"4bµEºw?øô@˜ëÛ?ìèêÅð¬ê?¤RiàGI?—Ö†"‰&û?…R©]A7D?²Ã+˜Ní?¡$ÖÄí?îäuØô–?•¸I©¶¼¥?ÂáD(ª?!Öæ1¥ãÌ?¡®Ar??•³8NZ3FGL J0345.1-2353@kEi_ªŠƒÀIm|_Ìï1À9Bn
Ÿ–3À;ªªùš‹?æé»áJ»Ä@{Ú\S=@CU_'òc¿âýږ‡Ì¿æë)ʏí¿æ2ًn€¿åš\Y""BAGNbll?ïM,S˜â?'~óg-qi?yþ'ÑÆß[?vT!ñ()?µ»6Wa?Žf̗JP?îZQæù×?«CÃ¥Jaô?‡Wχ8v?'Uƒð¯¡|?¤"í®™»+?¥fِI'?îu…JŸ?"q/Š2y]?)¾Ö쮥?rvRç¿2? 'Ëò©žÄ?Žš˜,ª?ë1xþM›ü?¯}º_NÖ·?›í~!òµ?"ç)	€?¿x؅L£t?­§0¡»e3FGL J0348.6-2748@l1~þáÀIr¬¿ç<À:ëWÒNíÀ;ÒþÈÈ[N¿œ@2 îÊê@ƒg5™?@6Ÿú0Þ¿æxxi?¬
¿ã›åGO¿ã¹Ý³h¼q¿ïÿÛå:úAGNfsrq?ïk2êPK?§§S•êý?wt×ȏÔ?"XTÃ̯¡?‰xã åŠ?àVV8?î͓ͼ?©yA™¿®Ò?÷iÙ÷ý?'ýA€ ºà?§rèè¸öM?£­'¯Ò~?í"I¡D]? ".NEŽ"?ª'‹¯†·?—yAö'Ò?¤fXÚ<3q?¥SÖ…?ì§Q?Qç?¤×ç
$Õ?"ÇDÅ`Œ?´b–
ØT?µ"¤Ô-ï}?¢a؋Å{3FGL J0348.7-1606@iè¾ß¤?æÀGË <¶jÀ9wÅüÀ;Ä	Ñ:×?çt[5}2@ڗ.u0@»#à)¿àx7YáÀ¿ç'fÈHr¿è2ee4¿åH6¿H™'AGNbll?ïéol‡'ä?_Œžÿ!²â?T
i²\?Qlm²>É<?Y–㐅?U}"ýãD´?ï<û{b´"?"ñº9*Ž}?lÑG7'¦i?pÁi =-?"Æg¬¹µ?'÷Ðý±¤?îÕw0§5?Œì¨5M>?‹®€`ˆ3?€ÃT¿'ÿ?—ÉBªßÕ/?'kw"h±?íQc¦@{¶?§™è•Üæ?W
åaDD?‰zJæfÑÀ?±_ £Ñ6?¦FR2>`3FGL J0349.2-1158@i<c>ÿPÀFÞ-ÿ틉À:.¶(E™gÀ;¤¬§"W`¿Ó7‹¼%#•@Qð/¨d8?ûÀ
ÿ±¿äW̍ÀP¿Ã1®õ\Ÿ$?¼~=Ù»ƒà¿Ø䢃šv0AGNbll?ïÝøð"?sÑ\¶¶Ì?"òŸiSõm?"á¼µaŠ,?pkòõ±žq?s@ÆäI?﹝ÑN¢?€gN"mMZ?Kõý¨ì>?T
8Yw­R?²W£'l?~KỸk?ïÀÿ¸F?ŠëD8M}?ÞšÁI<Þ?o–#gBÊO?–8'¨Y8†?†½§÷àf1?ï'O*Ze?†ßåB\…¸?W¨ÂÎÖ?%Ô{ˆ??†öÉ?†ÔÀx7;¼3FGL J0349.9-2102@jÌ¡ á÷×ÀHƒ-••À8ÅQa£ÊÀ;Ÿ>øcSŒ?û¨:üÖ)î@í-(­Z@Þé	nh¾¿àzZá;Þl¿èù›âÊ¿ëòPË°©<¿ïù¤ë¡#AGNfsrq?ïח%¶.?r-Lo§®?g"ýi Œò?m£ÆÝ'¡=?`ãÜà±]E?aùlù?ï¸6«Ô=´?' ¾\EÍk?S‡å Y\m?dGwÖQO?°ÍÊÎÎ?€
Juï:‹?ì½þCn؁?¦²æ€z¥Ñ?±+pqʶô?¡Žñ»jã?¡É:å}
?•iM:BÀl?淋®Í¸²?‹e)Á#ÓE?_Óý9tø?k<3€äe?'1ê¤Ä?‰[JMÖ3FGL J0351.1+0128@g[@îÙÀCÍÿÒ³—À:qbBë7À;‡»DLÊ¿r4G9b
@
›mrÊ!ø@r*ßý ¿â®õ惿éì¸
Ú
¿îùW'8&b?éM°&±AGNssrq?ï9Ú/¨X'?¡˜ÎJ'ý'?e~IºÑ?DõC:?–ðê]­? vÒö÷~?ï«v•J?Ž5\ðü?V)ú¾ã¨?v0]Q1?'_ÛcÑg?ˆ¿Q˜°¥?í—g	¬? om×&'?š—H®TÝ)?…ù[l==}?±rœ!ÓQ?œ3Cì=ty?ï^"tfî¹?—ufñ*V?<))Óã0?\֘͡†ù?"ËËҜ?—XfÉÍ3FGL J0352.9+5655@b9ø -à@½¾`Mr¥À9¿aY·+{À;j¥.ùÏ?è
~A4¹×@
ßôA…ÜM?ýT@ÿ¤n?é_{Ò£[?ïú¼3Cñ"¿â2	6¬Üº¿Ù£}`Ül[AGNbcu?í[¹ª"Ï?³æ¨íkT?"Òߧ´cµ?—­<60?°-zÄþè¡?±cpäK8¸?áUYÆdXm?Ӂܔm-õ?ÂÀ1¡F:Ü?ÆøŽœ˜ON?Óõ3¢"1·?Ð0-Hë?묂Vs?¦S£Ž¦?¤ÛL]>Ô4?'fÎnò}`?¸.G ¸2R?¡¡¿\ð­?áÔrd€A+?Ê#~2±	0?ؙGßò±î?Ì<CÔé?­îš¸f]è?¯'ý1Î3FGL J0353.0-3622@mÄô@¯¹ÀIUøØþ3À:w™Á݅'À;®0Ô´!Û?¶aš
¸	@Ì<C¨ p?øÚu!??Ü¿ïÿVëQж?ïýÍ«øty¿ÐGЬ³ÛB¿Ê'H/wDŽAGNbll?ï÷Žþ{?\!we\t?ìØtº­&?^aG?NÉøùf»…?[ÂÜ6"\ö?ïµËƅ­?Õž¯Jf?QBÚé-?l5
²í8@?€j8&7i?ŒAûwÂq?ï I°¦!?ŠÉ¡iÜ i?'™Úz2ò?|šü¬äIJ?'ªOÜ®"z?ƒÜlãÍ*t?ï´ÈÄMÙd?ˆù0¯|ã?E²0í£°?N"ã[Mž?r«ì:Ì·?ˆÆ1ÕM8›3FGL J0353.0-6831@q¬' ÄeÀDcX R…ßÀ:;Äõgö‰À;­…¨K
E?°QÔ
°g@
èlXï
?ùÑ°Ÿ¶5¿ã?^…zˆ¿Ýå‰ïNú0¿àì7¶(¢?¢¨´"œ¯¤AGNbll?ï§PÝÎ?‹ÀÞò[ªà?9Ö^y¥HI?7T‹I»?…m8Ô¿N?‹"uä¦ä?ï»ö°Õ™?zMæ)2rø?N
—h(ï÷?VëÎúOé?~CTÒ?wÆéÏû?îŠ9f-»?'´×h\´M?Ž%AëÞë²?€cQ€#‰?Ÿ¦2Dm'Ñ?‹F0ãK>o?ïU€›óÏ?"œµ—UÜ?1Ÿ1¦"†q?Búښ¦cÇ?•	oÕgt5?cO3tú°3FGL J0354.1+4643@cGŸfb5À«
–ìÀ9·ß(ë²À;Y
W—Õ¿'ÙK•'"f@iÆ@ì"M@
ä?Z2ü¿â'¸…¼Ì¿çÏNK+f¿â¶ë±`Ø¿æSZ¨m
AGNbcu?ìô²U»b?·LÀyç:)?zÌÅh²l?w䴚l??¶­®(û™Í?¶àˇ5?êŒÙ´M?¿½âf»Ö?–¬âAj]'?œŠn™Ÿ?Âöüæœ@?»ð¼BÚ?íMµÕ0­³?ž"#6~	?–ê@ˆ]bl?ƒÁbØB1,?¯¯'hÆs—?˜xHP¶Ýí?ìšhi·&i?˜ ¥oê'?tƒŸ*·'‰?i֐Ö>[	?¹ä'¿›T?˜;‰Zm­·3FGL J0354.6+8011@`Lþ?5Ÿõ@4¥_ yˆÀ9†mpEã9À;ٞÞ|øy¿âùͶט@Ld×pä@ü?_'`¿åÝë«_>Õ¿ä>ñ5'g¿äN­i"¿é ä´AGNbll?ïó3Ýl Å?m½¨N†?B¹ûVÚ?NÞçÎìQ?P•è)	[?iÎU¸â¬¥?ïÒhä·
×?zÁMÇ#ñH?^wd°B4?eDܐm~»?n[i;ó?u¶®(à©F?ïK=³nÿÞ?"™8ßaà?~"i÷~µ(?u…âõ+3?Ž^(€­ø?€oÞHkïa?ïüx]Þ<È?C2STz…²>ÖpV)®>å+efˆßØ?;ãOµÝf?C a']ñc3FGL J0356.3-6948@q¿÷À*ýÛÀCéUÿæՍÀ:C|»<'À;ßÀãŠ~tÀlÌìW@U<µ'ôd@<šà–ƒ:¿èúJÉÒÇc¿×Ù­w"œ¿ïÿ׶µ´,?ï÷7ã=ŸAGNbcu?ïæÙ»p'¥?nk0Ze·?Wÿö·€?fÖÏ·}s?ZL'gZ4>?`Ëªž?ïÆ®Ê>´k?{œéøw?GºÍ6:ˆ?P@fqƒžú?y±A=?D?yLĄ¯?íý#±3Ór?•çÿœ-P?™f'ó\‹?ˆ+©Œø,?£z°óˆ
?ò²e›D?ïú›®0??Pªâ.>¯üäßy>ÖðÏÌ,?EŒˆáë?P²d‹ò|3FGL J0357.1+2325@ehß½jYÀ6ppCßÀ9ü³1ñÔÀ;˜Ûmy€¿ß>^Κ@
¦•°ÖÍ@JÀŒ}¿äÆî–Ì	Ù¿ì—Õ°\¿Í™Sƒ_Æd¿Þ='7äYAGNbcu?îx@²ש?¶1'x5Â)?Ni1	†èð?_4€ò¾ ?¨Pià?µÝÌG­¬*?ï vPDÉ?†ºð¾d1O?_@'pçU?k"µÅ5»?ƒúYÑ«p¨?ƒ3&`i?í¼ê:<êG?›z'ZFƒ&?ŽÿÅG?{šcSþ§f?¬qœÀ	Û?—~ƒ¹Î™?îÎ@ù2¦ƒ?'DÁ«Ã‰?0DÈ'C¹?=$~qò?¢ûf܇¥?'@ð
3FGL J0357.1-4957@p+i€,
JÀHb`GhtÀ:+à¤&À;ù)CÆ(nÀE¦}X@V†´åzn@DŽ*GQ¿Ý!Œ@hâ¿åwºXáA¿Ù¤ZŽ}¿à¬$vAGNbll?ïùyΗ|ý?G§ÎNî.?÷Ú
™?.ÜË`?H'$k¸G?FmYÜé]?ïý¨ì¨'?~ŒäL¯ôø?FK;í )?OT?<eé?{WÊ.H'?}Im|?ï8ɔl?°gàCv©?|œ>ȹgÇ?jYԔ'?'×WD%Ç?|öË?üâ?ïÝ~yë…?m²@¿v)>ÑjN]ð>ãhbNc?q<hvØöÐ?m®2–~Ów3FGL J0357.9+3206@dX6m
JÀ/ù£~õ©eÀ7q=Y&ãÀ;="Ö¼@üFØ
@ñˆ\…g@"Bè\ö¿ÒJÿ5]c¿ã(vÛmhR¿ì§nœJW¿ïj?©¹!tPSRPSR?Phya|j?]rðÆ?ïèXïjK?o&óv¯?^å§Éia1?g4U.|mt?FøˆÄ:Y?`õ¨z(‰?ï;7É®ç?¤y\û~?žçéB"H?£¡KÙô[o?Ÿ	Š 
¼E?•<6¬*?ìv3݋Ð6?¤'p—?´‹þ‹ž>?žË7þ<ð?*%
Tu?/w¸1PW?ïÛðˆ&d6?r†ª£'?q6"š-,€?r$òÁâ#3FGL J0358.7+0633@fê}æOUÀ@Çk 	ŠÃÀ9EçbzH›À;s® 9[k?Ütëüà2R@ØJl4܁@É •¿ãþÚ®ŒÅÌ¿é9Y¤e£¿ãu5ÀØß¿ïÿqtâUAGNbcu?ïú-.Žrò?C¸4mÜ?€Ó‹zq?¶Ç"Ø4?E3«ÂÊÚ?BàY.¾*Ú?ïrx¼in?Šåð•@™?dô¢?iHˆô`Õ?Ž$̃óH?‡®‰Â9€±?îü<a¨QÙ?ˆ¸L÷ÊñÆ?ŽxaµoC?~veNtƒ?'<Bðl
E?€Þúl«c	?î"ãÒÝÛ?œ¯(öKÿM?vs¸kíw?ræqÖÞ0?«XTsr?›'S²»p3FGL J0358.8+6002@bàP7P@è‡@%´ðÀ9…З]À;Nâ~ú?Ý3ÑÏÒ!@)ðÐq@$ˆÿÃo+¿ãØÑÂ؃¿è²‰"p	¿ã‹·	RJa¿îXQúøÄAGNfsrq?ïƺ´ùu\?uÿ(>éé±?UE-Xáo?R™'½!5R?wQZ<ok?té¡Ý¿?í¬cŠÔ?³'R2ñƒ«?q°ì3îՁ?vÍI(æ0c?±Øpp|	?²ÙÐvë¼?íKʛÚ?žT·sx?¡znÌcŒW?"ä;Àh,I?¦pԉÞÓ+?"+S<—Þ?ïŽîO³›Z?†×&¨?C÷œÚ/ñj?LžÉûmäü?‹òEv*²?…×Ý	y>3FGL J0359.3-2612@kØädIVÀH!'	±À:"QN"¹À;Û4̐fë?Ó½I¬ÇHÔ@
Y9Ìö@Œ4ÿf'&¿è‡-á7¿é£¤"ƒç¿Ó‰J†áÛþ¿æHðLÙ¢AGNbll?ï³m帽‡?…Y6ø4?1?™Úm¹*?5DæZúŒ?'š‰Âý0Œ?…²áBñÁ?îü§ýDhŠ?¥7Z"!45?o'@aó?u:ãÊö?œxßTjâe?¤WÛµÿÿU?î[6åTI?'‡µea?‹N²–]4›?x¦Õ¯Ð¤š?£xå$!¢?ŒÒtג?íU/chˆ?£÷yçF`?p•–è>ó?tº
ç=;R?´M3+M;?¢nvBGCB3FGL J0401.4+2109@emÌÀ7"À7UH¿ŒrjÀ9˖‹È¿À;‹³ß•ý-?îjÌÌÒJ@á㇤N©@ω REr¿â½¨ë¿áŽ"Ç̀ô¿åœ,4ÖZ¿ïÿ4`tAGNfsrq?Ì£1È&^?Âß»"vKm?áÜ)wÊ·A?Ëã Koht?Ëì(X®Äï?ÅVOlþ§?ǧ†ÔfG?½íû>?ã'VvN?ÄBÌÔ¿L?ʸ;S\ƒ?¼W1†%ó?ã3%h¥|Õ?µ–pe†ê?͓†@bÎQ?°$Wz'Nõ?şä>[?­'—üy²?ЍZÜÙí¾?±;½{Dډ?á;YkjÚþ?º$hg¨!?É÷䘠¸‰?®FóÜYv3FGL J0401.8-3144@lå7?1n7ÀHN‡à3±ÞÀ:V"ú¾À;ò·1Z?²åäÃ0
[@}ù?œx@J‡™xb¿è"Ûs¿çÔÔxñ6¿Ö¢}›Ǩ¿ë-:¾AïAGNfsrq?ïÌ6·Îæ?wäCÝî¼`?@žU—â?A®ªiëãB?wáðW'?+?w$›wå?ï'MûsU3?"ÔÊþm­Ê?pÒ-lí	Y?t¬¯ü, ?–áµ6Z^?'0ÆdýËë?íÇ.¡p"?â>·Ô¥)?–;'vj?'lò—œ*?¨‰øg5"ê?˜	1·%¸•?î>\"DX?š¯ÔÐÅ2ý?q[u€Þ?ood¼¯Ð?©óWï+žÒ?™Ž'î±3FGL J0402.1-2618@kä}sÉÀGÓõÀjÀ9ø|]H°À;·ßâSG?åËWw"½ë@‡õ!ªŸ¦@ðX•m?ï2î>âi¿Üc‰¨ÆïN¿çÛ¸M
û¿Þ¿9€:‰AGNbll?ïgo"–dh?–•#0›'?v÷3!Òzä?'¶ïdÐz"?Š¨…I}¨Û?'¢gÊ+Z?îÙ[÷b
A?£¨$
^mˆ?yo'o9P?ƒóðIß}?žx·Ob‰•? €ÈèîI†?íVK9{†?ž£üŸ"^s?¢K]cg-œ?';%æœÓ?¨Oïàjx?"7œ
â?èæÜãJ'ã?»›<ËÈR<?°©åæ'?­Oö¿þì ?Äb7âàé?¶õqŠµÐI3FGL J0403.7-2442@kž¤_ZÙjÀGzX`fÀ:'ÅÁ?ÐÐÀ;ö2 f<u?¼#$Œ;j@ñÈS{½@ò`À48¿¾–û\_Û¿ë¡ÃBE°õ¿ÞýϦ=cZ¿ïòÂómAGNfsrq?ï@zûp©?Ÿi{¿¹ñÜ?p´&$n±?}\v}Œ?"¿óˆaÂ-?ž¹¿©?ëSÐÖ®c?¹lºLÙï¸?¤×/²æ?¦¬Ì«xuú?ºõö2þµ?³Ãͳ¼Ÿ?ë"t­aJv?¦£hÝøÕ?³x­Î©(§?¡Fv_Õ?³s¬ÆLƒ¬?ž0<uø4!?é"Ç}Lxj?±ùâäþË?£ö•/jÖ?›õ}cÏg,?į<¿ƒ£?°/þƒš¦3FGL J0403.9-3604@m·{€©Þ‹ÀH;Ã`<€ºÀ7/.g˜À;>K֘'ª@Žƒ¹Þ^@FG¤5)@¬BIхC¿â¡w¾ji¿è ×ÌOñ¿êPEҔ"S¿íÈ%?¡øÛAGNFSRQ?ïEd×ì?¦VqpZ¾Ì?"ÿ€ËôÀ?¦%™¶¾~¿?bäàTÈn"?bÚÕ8¶"?ïÇT•´ÛÃ?~Ȇ›?OÙæ;4G?rˆ-¶Þ?xZx^+›6?w>KÃÑ#?ëv¾¸VÂÀ?ªùê+9cÂ?ºÞt2ðŠ•?§";RøÏ?¢×,²¾×?š''RãÉo?ïé9j_Í?wµ.+á	Â?(YˆÚc?GlÍwta?e>(ýŒM?wr	OèÛ3FGL J0405.5-1307@i¸ߨq¤ÀER3çüÔÀ9Æ$PA`óÀ;Èi;,ü¸¿ô/Þr¾"@öÉ™"{@Ä<€L¿âËK-ƒyz¿æŸÚ÷e…I¿áa¯Ü7_#¿å³` åÏcAGNfsrq?ïï«`çœ6?cB±˜¬1§?Ҙ¿ZÃ?wÝ!¸?_l¤Ñô¬?cÜ»j	?ïŽ}s•ž?x¶@ªJÛp?G/%=¤u-?N'›nf.?z;\ž€¢?vu'SL?ï.%?Š?'ê~ãg?xÈ?5ª?d›³Giù?"	YÈOé½?€%
#È?ï͹Ó~Dv?qzöп{>üS"Ó»¡³?a…Æ©G?y¬
	C?qm5;sËZ3FGL J0407.1-3825@n(*Á	J,ÀGìè_ÐJ0À8î÷™ÿñÀ; ÓµZ?ð¡R¥ê4è@õ5`Šz@.âôV¿âŸaþü¿æ=U?;n¿åp»ÝøTv¿ë ÂJñIAGNfsrq?ïÌB»‡Ê‹?q`S(n?gG©6àµ?böîõq¢î?lušèþ•Q?g^c=_x?ï˜îN"‰è?‰½À[÷Ҍ?Z}Æc@Sa?aÝ4‹`É	?†t³'u{…?‡†£GÙ_?aq#ß?•1¶³¢²?—Ã
dÕmþ?Œ¾Ñåœãô?—hIm&?‡,/¬OÜ?ïJãÓdv¨?"¡´M~?bÁslR>'?bío­=?"KW%æã!?"jÅGt3FGL J0407.5+0740@fý-`ûHÀ?)£?4É5À9\¨\ªûÂÀ;nNá£1¿ñÕ«}Ç«ü@Dõvºš@…¹'!*¿è®+£4I¿æ…Œ™"r¾¿ë^BØ¿À[{26šAGNbll?ËùÎ?¡rD
3ø.?{´C½»•?"
p2«¿?—@Ú'Wb?žo;%zÖ?ï©gÔáS´?Œ—¦~Áàì?W		áó\4?hÄIÇ8ˏ?'Äé‹l§w?‡Ú_úâ?ìÇ7C[?¢]:Kÿpl?Ÿ³•…k´?‹r€ê0[?±Ùb•Âø?œoÓi?îҀæˤÐ?™PUàíQ?1Æð¡t?@7áawd?¢´c²¤Ô?™Iqד³3FGL J0409.4+3158@d–]¿Î·‰À,ÎRAtÀ9ÿ°ŸoœÀ;‡yÎøö÷À¢ëý¿‰@S¿[o'@û¨»w¿êX™|ÆØ ¿èžô'%Æ¿ÓN¦Œ-¿ã‹Õe"¼AGNbcu?ïΈߛW?€wlv'?@Š[Sù·?@Óån¸ãd?vªDÈ•Ã?.£àC?³?ïºy+Ž0»?ƒ¨êhåÏ/?TîCa#‰?bH/=<¤•?}‡ÙxYp?kæ!Ÿê?íèeb@?›ã@òp?D´ûõÓ?|Ê‹'‰?©¨'¯cž}?—ÁDì€Á´?c
7Ì?‰ù¤¹&î>Üc™'ó_ý>ðœõ?Ú`?ŒZÊ?Ρ?‰ñ›yø3FGL J0409.8-0358@h{¢ÿ‰;ÀB¯Ø€_5ðÀ9n93't¹À;‡#µîe?ë\˜1e@WtßP)@"< DXŸ¿ÅéÊ A‹]¿àuñ—ë¿âÏòU¿Çx¿àŽ¬£ŒŒ–AGNbll?ïÅ$AY1¸?uUßÑfTß?f¯/Î÷ú?gåg"·=²?rGÎÿ¨'?jþ9|BÁœ?ïS©q0í½?ŽÚaE«§?jºúúþ,s?nèÉ¢<¤ð?'3rz''Ò?Š¿¸¥ªe?î$Í¿	7¢?—d(Åì?ž{IÚ¶c?µÙIéّ?HÌÔþUk?†¹²ëJ"?ì[€ ²8ƒ?¤YÈMÐ*?w¢´ó^{?‹3mg5\Ã?¹5£ÏÐ?£jºn3FGL J0413.6-5334@pm#@ˆÊÀFR ÿ¿h`À9:mæÎÀ;¼À2Š–Ç?ÒGp²D¶=@¹Zîu@Ïâ_[/Q¿ä"9¿äEÕwŽà¿éH0s˜ÜŽ¿Â‰,2§¶ØAGNfsrq@?ïï×-l¢¹?Xíò—C®?:+ÑWpK(?9gDôPî,?YÆ°ÐÞ~u?UÖ.¼*0Í?ïÈ¿¬ ?yOP4Í,?B!l:¤?Fû²oIz?y_tO¼)?x#=¬?î÷éV­#å?‹šd&¡4½?"ièˆ*ÁË?v+"þªÅ?–ÍàæF"f?†yùu?ïónõOÎw?`s0pÍZý>ì,Ú¹ÄK?^-k|Ö-?Xé½0­œ?`a¥øêaj3FGL J0416.6-1850@jÉ{¼¾bÀE/0ŸÚü:À8þ,"	7À;«kÙlî@¿¬=¨7•c@Á'eé>@¸áß®{Ô¿ä€ÚB×%¿ã
–t 8Z¿è_
Úyˆ­¿áEÀDbDAGNfsrq?ï털^?`>€&'àU?BH-t¨?C;Ž¹ˆPä?[ò뮉o5?[dQA)BÈ?ïÀTüDƒ?|ðYØ@S?I©ÄIÁÑ?T3ëßFŒF?| IT†]â?y†Â£°ý?ïæW¡B?ˆ»¼;ƒ~J?…>ƒoáÉù?v–?fJ?•Cý}òÐ?'x¸¤l|ä?ï»(ÚLÞu?€º'ñÉ|?+¹Ú¹óp?2bքnÌb?€ÆåY]{?òX) -3FGL J0416.8+0104@gúŸDÔEÀ@"п "`À9‡Ûk=À;Wè°X"ÀþHDè<@0:/{Ä?ûë©ÿ˜Q?éW
¥—̿仝‰'&¿ÑmE;Q¿ÐàP7OøfAGNbll?ïó÷xeÍ?d"ø"Ç:?M´G66æ?A'î`?Vl4˜Áñ?cÎ'º~?ïÉ×8³i:?wlOF<?Hf`$©Ìþ?SšœŒ¾Á?x—¡¶)?t§x-/
?îÝ¢`ïÒ³?Œ¶«.af?…(&Ö£™?wÔ|8e³ò?™· ÕWÝ?‡=òý›T"?ï¬yrì¿%?ƒ.®ÊÀ×>¯%¹Q>ǟî6‡Ž?"á&­ê1v?ƒ.¥<šò3FGL J0418.0-0251@h€§ayWÀA"@f!À9#'RÑ^À;‡JaM!ò?ïÇã_û,@=×{ýQz@¯'ÿÏ-¥¿ç'üÏ¿áçй–d0¿épN[$O¿ïÿݹë.ôAGNbcu?ï֜‰‹ka?s"m@uP£?p؇ˇI?qSÄÃwD4?Nɛv5*?P-ý:™'?î¯;!?žÈ֑p€?'êð¬.#?…\ƒ¯MÅJ? T‰KÄBq?˜1 Êæ ?ë®xß ''?¦Sp4¶Ò?¸OF˄®~?¡þýÛÕ°?¤yänô*?'ò¯žLHG?ì»j\€?¨³,Îc˜?¤Æ'ºœÁæ?Ð˜hlÛ?¯‡—¤]v0?¡Ò™;7€3FGL J0418.5+3813c@d2`c'À!N·@§[À8סíûñ~À;4'b"s?ð`ãD³c@Ðü&Å£@K7GMœ¿çՆGqD¿ëùt7	'¿èˆ¦0š–^¿ïÿÒ"¢kAGNrdg ?Qe?"ýù²'³´?sù™÷óe‡?xÐ÷•"¯?€"R½ñô,?'«eŽ5ÞW?Õ5Ž–ô"ì?ÌWJ‹3¹"?ÐàYDÒ‰?ÁÂÿžË(l?Ùê$9ы?Ǒ2€uˆ?ë'¬P?u?«.Êh<
¨?´së>û
?¢c_}.g?³^'úa?ž"®ÙcŽ?ÜYm"½•?°•5Ø°d?ÑO00›^Â?²_DEÂÒ?ÒW±bAã©?´xüÏÒùE3FGL J0422.1-0642@i@lÚÀBÛíöéÀ9®°E­‰À;¹V¢¤W?易 ûðs@Õ˒@Q†Àyt¿àÖ.½Ø"*¿æ){þS-¿è§´í]&¿äj"]Ú£AGNfsrq?ï2"\d·è?"Ͼ73ßð?Šî|ßNŒY?ŠÆÖeºûï?ˆl¬ƒyc?…ö@Ïjä
?î|B9'ï?¦,¬Ó˃?ƒ
Q¸™™ô?Š{)2?£yJÎ@j?¢	4~¼Ö^?íÎ~–ÈB?˜#´.^žÔ?š¾Ó½ž?‰Á8{…¾?¦hÇ©?K¦£¢HÑ?ë¾}ˆÄK"?­Ó.Ùµ?¡ :PAï ?™9'¸ñC?¹;ö'¼«ã?«ö(0 3FGL J0423.2-0119@hi#ßm¹AÀ@5ߵݝÀ7‹@ºs,À:îﲪâ—?õºX€õ‰@%@ô¼Õß@ž`‡)T¿á×ù}Ò59¿åwGø<<F¿äÝÌ_¥¾&¿åÃ'Š¼ÂAGNFSRQ?ïà")Ý_è?g$
gé¢o?3 ¹â¦–Ö?4ð²ŒmÓR?lø¾æKEƒ?fÓ$‡O´?ïÁû[Jè?zëÖ!7¦?M0ÕÑwô?S›Ÿâ˜‡c?{\N 5Ýv?x÷ŸÝè=?î«Æ6
?"ýÌ1ì}?†Jáí·×d?}²¯h"«o?ŸaÎ(ÝRÂ?'\£ùÚ^?—¡™Þ?ˆ‰8lxý:?%¢0qž?1Êßã|öâ?‡¹ÏŽ×Ä@?ˆ;±o"3FGL J0423.8+4150@cöX@žUÁÀÃßé47À8MQŒ»À:Ú¥ÉRÄÉ?áE9bã@«ØW—V?þC‡¿&›ö¿ä™˜¦eÁ¿ÞãÙ5¿ÌOąÍ×0¿áS#h¹0AGNbll?êñ& 4Šu?½óÅa€½€?Dd*så?ƒ@$Í
ô;?Ã''8ë.ï?½ŒvÃí³?æ`ú^Š|?ÍÁLß³?°	z¾
°¤?±{[Åÿyf?ÎwY&Îé½?ÈL݇BÂ?狅ã?"?³Bµ•áRS?ªmú«Bރ?˜RU%Ïs?Ë6iÈ16!?°qán­Z?ã§CiÞþÅ?º}ÄõÏ݋?'ËkÓCé?{Ô?הÂo
Ãå?ºJÈD1´3FGL J0424.7+0035@h2¢iÀ?Ëy`>.9À8'Ld\¡À;Iû_‡O?ÑïdöyÄ@üŠOú"0@•?æ¿Þu—''¿åsÿ©÷h_¿àSwa¥%¿ë/ó
åAGNbll?ïÜ͐§Œu?pÅ;æ?<°Ã5¿J\?9‰ßÀ%˜?oœVñ»¢¼?o;ùh' ?ö Õ?Š0s·éŸ}?b.èBG©?dì÷Jûî?‹ˆVú*A?‡Á‰ yfd?íÉ¦<âú?ž+`á¤xH?¢&N‡¯Ã?"úÄò:ÝQ?¤?Mª ¦?"Ý XõL?íó7¬e?Ÿ×àNõW?hçwIÞu?gÕ*ŽH ?¯>4…\?Ÿf>ál¦©3FGL J0425.0-5331@pbâ:¸cÀE€ÇßþùÀ9gCÁðÀ;ԝñ.ñ¿õåØõ$.Þ@Ùð5²"g@®ˆ  ^…¿ä¾è$/ùÝ¿äÔ7r2!¿ÜÛpí0£¿ëãAÄלAGNbll?ïs»@/[÷?'ž]ôé'??nÊ×ëؕ?tdÚ'T?‹^®~.â?I¡m6&?ï…)ozÎì?7%"¸?]'>e±?i¥	Շ3P?‹\`?¤è?Œ¸Ý—º?îDå%·Š?™@´¤+p?š÷à:'*è?%"Hî[p?œk{ãÃ?&ηôŒÙ?ïg!ÒòÃ$?‰¥P?6¢!6ÒÇ?DÏUK?'Á;"ÀX?Núlf"ø3FGL J0425.2+6319@búâ~@#…ïÕ"\À9Â*·c®üÀ;röq?Ù¾9½w*•@Ì~ ïÏ0?ÿme¾Ë­=¿ã—vå˲'¿èç	<Gaœ¿Üf9±~N¿…è¨(0ScAGNbcu?폄À?¶\8"pCf?Yiù¶(a†?ZQÝl.ˆ?³7Û&¥…?¶HÖ;&ÍÛ?íѬ
Éݾ?µ@gÁÐ?z·t¼¯
?ˆ8c‹Í—n?¯ŽP‹ßÎ1?´A!?íÓɔ¨Ð€?ŸHtݎ6s?‹gæJ ú?|Z]}¨\‡?«ém- O¯?›'¥ß
°?îëû½;pd?"¿½û>о?J3`³sQÝ?[Nã.tÆ? ×v©{,z?"À̃ ë{3FGL J0426.3+6827@a"¦°)(@*°°|À9ǾZCBuÀ;£°Ôcš¿ñ·O,´@ '¯€@Ò@!¿ã1i¼¿è3©a|‹†¿â'7Ín)̿䈺›"=AGNbcu?ìð\ðK'?¿¾Âڈ@?r½Ä@d;?t¹é‹Û'F?·Q<;Ü@Š?¾øÙ·_×?®«?°FñÅ)¤?w¸kU'?,p7?¤­Nêc»?­÷"t¤q)?íß*å $?¡Ìµ½c{k?Œ"t[È?zï#·6…T?«´©fÌ.?Ÿ"|'©Yï?ïW7|E?Œ7¯ÂÂð|?@B,€ß÷?B¢Ø聝?›"µ	%?‹áfKñ3FGL J0426.6+0459@gµq'lÀ<î™?׆dÀ9RöT…"À;T"K"bÑ?'Šò˜Ö~'@°Ü{š*@q1ßöö¿åxŸú쵿çê_5UÞj¿æDªøÍÂÒ¿é>!'}AGNbcu?ïÈbü¯™Ä?"6­Ý…?VZ9ße?pEO[ÁÖ7?v7ó0YÖ_?vþÇE©¹?ïpŠè¸Œû?+"¬±'?h€þïÈZ?h«a)	?½깘?‹ìÎʉÆÛ?îÀhwSØ?'ßU™äž?‹ˆ)7rÍ?ƒ&é*?š.î‹9Ëj?ˆæMXüô¤?ìt"K^ˆ?ŸIzœ´œ'?y	V0–‡?q!øa§Þ?ºĘ̂úS?Ÿ2ý›}†¹3FGL J0427.3-3900@nEg!éBÀEöŽ€`ãpÀ8»rƒ«ËÀ;AHð3Ú"?æ"Uö_Jò@¿%oü^@`;»²¿áÿfyJˆ~¿éç±(Ó"¿çµ'"?W¿ïÿGýUçÏAGNbcu?ïûÓsÕ?DÕE¨?#šF«s? àAŒqxM?='Ù¡Ë?Bu2m8À?ï†Æ¿5'?‰:òÁó2Š?[ÜóL´£?`v^ c`?ŠÒ±É?‡nð/²0›?ÆTaû?'5-m¯S?•}SúÎÀ?†ñèäÌ?—"µxñþ?‡ä·'
óF?íÙ싽Õ?¤3þg;êÀ?t1uûåÑb?t~t¸@)ß?¯Û"¥ôq?£›š¦©3FGL J0428.6-3756@n‡?úÁÓÀEÏàaÕÀ6jˆû¼¤aÀ:3Ám9Í?ù˜ðN²»@õØ •ŒD?þe@å£]¿Ü},ÈØC¿áC,ú¨¿ßì>{¿äŠI2à
XAGNbll?îOzLV:Ï?¬2¾ƒ ¿h?@ã­l ý&?L©Ñöæ?ªǞéÏ?«êbKf=È?ïËÀìžb\?xg–•ÂÂ?B±¡GÑE¬?IÕÆiÂHâ?wÉU‡Ô©õ?vŽ¼â´Í?蝃Ød$Ì?²C'÷¶e? Iȟ!^Ø?"ӊ1î€?Éw~v§?°°/óV??ïïXU(è»?iҀÿ¦]Î>ßï	#±ü?DÍE-ž?`—³R…mš?iÓð3u03FGL J0429.8+2843@eG¯ ×{|À*ôUÿøÀ9¹õÞ>YÀ;W'2ÂÊë?òÿÞÇöú@ZM{³Õ…?ÿiE pÝ¿ïœø¦ÅQ-?ít:!ín6¿ÛÏY*Nï¿ãf pMoõAGNbcu?ïhŸ¢K"?›<ï?Ïsh?¶Nª,Î?ŠÓh<Î[ö?"!émA5e?š]Ÿ§Á"?ëJö$à?ÇMê(
?¨Mnê²?°.Óy,Ì?»Ïc¦t?Âk("6??ꝡ[û[æ?±w¤*'ep?³ÀiÛÁ"?¡Ýd"ÓÅA?·RݶI_¯?ª'z«À²À?êt³ƒ£Ýì?¸^±éÿë¸?ÀÜëœ??´ÞÈ],Ú8?¨¡Wz°F?¦Èœ¶]¼ô3FGL J0430.2-2508@kóóà7ÝÀD "?Åè­À:•mºîÀ;Ï¥·µ
"?²v_ÛA`œ@­•ÇÒçï@‹ïà"?¿Ï#.LË¿áR»<	N;¿ç¿oA+n¿áq'ÝëXAGNbll?ïÙýQƱ?v[þ‰ç'?W¾ÏÖ«?f=àLA@?j#…Ã*JU?q66±a-?ï e
XkÁ?ƒkHÅ¡?UÄéÁ"¨?XÜ_h>I?….<L¬Ý?'
I¯÷=;?îÍ'âêm ?<ÝؙK?''f=š…?†¾kÂûž?"؝e®ÁY?'W5[ãNÔ?îø4õÇÀ›?'SLV1³?aݧ-†Ÿø?_7/«	˯?ž½¬aW­?'Ðzimr3FGL J0430.5+1655@fxV[åÚÀ5ªKÀ9B«×‰¿1À;NaŸWH¼¿á®ÅÁHh@Ò&Œ'@6†@ €¿äêG‹H·Ä¿ìRþ]Ï¥+¿ÍéY¨ñXü¿ÛšÝl"AGNbcu?ïëRæ"øŠ?døÞe£ß?-N"Yëq?/±¿§hq
?bØ0—hÂM?dFàÓ"Dh?ï¶êÙyš?'Ó
̃É?Vwqvìê?\æZÖHì ?~ì¶åwý?:êp??EY?–e{lÁnô?{pl$dö?p,aáR"T?¢§î*==Þ?•YD?½N?ïµ^o6?¤ºn­‡†?à|®õ\_?͂l%  ?žíùڞ‡?¡YZU3FGL J0431.6+7403@a``þG™@1\w·À9±{£aÀ;¿Á§ÕœÀfºó±h@
±Šî0×?ÿÐNI¿¾‡*…~sg¿ãš+Œ°a¿Ûf¿ÕÌ€¿Ú@`"ú¯oAGNbcu?ïj~©©)Þ?œ+LEÒyp?aì«ÊÏåî?`›'«k—?r•Q€Çƒ?›l-R䔙?ïr.²OÕï?¡¿âyé?dvBô; 4?j7"ÃQü?ŽV®û»ö?¡vK¬–Ÿ?î(OUÛ¡Ç?˜GGBq?"œgaRk?"8 YwžJ?£¬Öñœ®?'䌺õW{?ï¤ä¿»8,?Um6!D?ªtoÅÒ?ï"zg`?†ª%œ²…R?ƒ$8ê1ñ3FGL J0433.1+3228@dûá`؇ìÀ$Þܾ²W×À9ôwa`m(À;ûý<a¿ÛM¹ë¸d$@eýua+?ÿ~5?|푿äq#mÑG¿Ö¸ŒÃпàDe°¼~¿ÊÛk‰n†ÏAGNbcu?ï{¼b˜§ë?üïh?Pm&‡¾†?V"þ¯A?C•
¬?HõËK{Õ?層¶/"?¡ØJm²9?hÂi¥=;Ü?t‹ÊìüH?™2›T'eì? 2ŸcÐIf?îÉ_2TX?Ž{¯ô¼ì?ˆìW˟É.?xdbÂ
ä6?š]íÏ¥]?‡8.'¶ÉD?ï}§ú"@ ?Æú€Gw?&!¸Ž§b.?0`¶I"oû?½>Z­g?ªƒ#¦ÿö3FGL J0433.6+2905@eQŸÛÒúÀ)3UÿæՍÀ7胦MàÀ:ÑñËu?æ(Äwò3@Vmrõ@+&`;ÿà¿Øk®h¢p¿â-ôT"¿à+=ðÈÌÚ¿ßÎЇ\$AGNbll?ïã§ÌRÙw?h¹âӟ¥B?*­G5ìC?0÷¡ä'U.?j­_9Çț?h1^PÖ³‹?ï¶I¦Â?ƒýä®(]6?VRèåu?ZOOšR?k³²e'?'O­ï'i[?í΢¶W'²?Ÿš¶4?‹31å
Jq?ƒòš
€?¬I!C'A?œO»|?ïõ3hÁF?'²·¡«êâ?53ºót
c?<"þò;?ŒŠ§?'¨èS¹¬ª3FGL J0433.7-6028@pí_ôöÀD'ï¤hÀ9*ÜÇÔÀ;É'o°'?ãód»|ª@æ'M@–?Çì¿Ý&â k¿æ$³­ZÛ]¿èØ7»x¿ïþÏë݀œAGNbcu?ïø=oIð•?Hk¹4ÜÃå?6߯×^/]?8ÛûÅagr?Cšj쎓ñ?A\Ë-CÌ?ï³):E¸Ÿ?Y±_ Îk?R[Ú_$5?Y)	?€êO3Eó?'ÀTË?î&ϙ)³ê?™Ä´t¢›?ŸË5^Ǝ?'IñMÐ#?›Z×|ô¬?",—¸Î?ḯ|›ë'?}ezɋh]?CMvžóu?K¤zFÁˆq?vÕ¡6Žt?|eºyÇRK3FGL J0434.0-5726@p¯ 6mÀDq™_·ö|À9óÁ¯bYÀ;ٔ¦ë'´¿ªù[?ÿç@'Ùv©T£?ÿú•ÀF+³¿ç;áVûi¿Èx½Òš'o¿äX"ƒv±¿Òé`VVúAGNbcu?ïõcšÇ–?[z^ÉFaù?3AÃÀ/2q?={¶ý-ØÚ?PhYÇÐ?W#1`ŒÀ¯?﵆'=ó3?T:BŽô?LݵÞB?P‹—ÀÑ't?€ÝM•*5u?}˜X^ÃJJ?ïLq`}¼?Œ$&®z?…º Gõ?'ª™•œ?'9a¯õºÚ?"N!•£Î?ïœð¬sI&?«W q~?AònÍÿÝÒ?D¸äg˜?‡¤­öM¸¦?5PH¦C3FGL J0434.0-2010@k8
¿cíÀCx–@HÅlÀ9×
bY'lÀ;Å
ÎÜd?ðz8ËxŽÝ@m³Òê@–!@l³?ïù\œQôƒ¿Þ³4²‡¿æõb!£ò¿ê#£7AGNbll?è‰å¶ a?ĄEµÖ~?ɒSQ/Ìi?ÕEzD%ù?¡aÞÈR?£|¤½Ú1É?ë"?ˆhâ?ºéX¸#ýç?¨á†ŒÂÂÐ?®'Xâñ_Ö?¶õ@yCWŠ?±
íX½[	?æ+!âª?¶é‡Ôh$?ËÓiÁ £?³Å³ÚJm?·#Žãa? òëÖÇԜ?ä–^zÃ.{?Àk8íaÝ?ËÓÈ@¬?¸P°m#h:?'²õ+l?¶ìR—Fñ3FGL J0434.4-2341@kć rѯÀCõöÿ¦=íÀ9ø*/~rÍÀ;Ш•µßJ?äèþ®òf@{'Õ‡ÜX@ÃÛËÍH¿à>+•ì¿èæÈtVÉ¿ãÿ©²&¿n¿ääµ
_AGNbcu?ïO83Ot¥?"QÒ¥åBF?eÓÜߧ!¹?iã"e'¡?"^}ú‡C?'Iè/­-?î­i	¥ëÏ?¢P+Ʋh‰?}ûŠ«[Ï@?ƒ$®/ Å?¡iþ5É?ž!£m??îå+é¤e?—ý³(j¿]?"}Åh5™Œ?"5áR ã?¥BʍJìü?'L9·\£?ì{S'Ò*?¥Èu#úƒ?¼`nV?ˆ¹ï22¦T?·öKf]S?¥Å
ÏÑ3FGL J0434.6+0921@g^­@ªêûÀ8Ë@—ŸÄÀ9Í
eÀNÀ;‰pà<ìÀQ4MdŒÇ@&`ú–´@êè CZ¿ç™ØÕTìӿُW¿Ûu#¨¦§Ê¿èÔ;D_ç'AGNbcu?ï§î{{è8?‰(i¸(V?bGÁ撦G?eÂëd(*?rp§aH–?†ÑžÄBÂ?ﶫ®~.?€>?X™ô‹\©ù?_ED§üu?~ƒ«ž(>Ë?{4­âz?îM‹>…ƒ·?˜3d‡·ëÔ?"DJ."¡?ˆåù'®*?¡'š³+??å'r°?ïeÉJ–¨v?Œq–òËtý?XkȒMß?2Ǐ׮ùƒ?"(~Ab^Ð?ŒFB§¤à÷3FGL J0437.2-4713@o«˜€"åÖÀDüsßË­À8¿qw; ÀÀ;Àîû.	@šõº+àY@	«¼üK@ø/M˜w¿Ò´JÀ²¤¿är>Y_ W¿ë·D)Јï¿íĬ妸fPSRPSR?‰ýU1ë
j?'" Te~?ëø!¢LS?ÅèƒitwJ?¼ÿHG`z?Ĭ5$†^æ?c"ÝŒu( ?v§+dYÁ?íRð¢"z?¾ob'Õôq?·(ÁŽˆ2ô?½ïKH'y¶?º^B"Ÿ9?¦µ÷ÒV?èÕ-áÁ˜?°ÿÙԊ¥1?ü'/*?©XJènµw?EÇ(ï(ñÙ?Nܨú Í?ï»>¨÷®?y²3§?¨
Ÿ
K?€lã0"I"3FGL J0438.3-1258@j;4 -œñÀAª(CìÀ:/rq6¤À;ÀlÄNy¿Ó'èxWˆ0@ú¥>hp'@Ù f|â¿ÞAš»>¿çÒúdúDn¿°pN$XØg¿ëV°j¸ÒçAGNfsrq?ï€øÙ4c?"d0M«"¯?Vü9ºáqL?WÆLè¼?ŒâB{‹Z?"ÙÑÁ•8Ú?ïc†õx¸?°z+üdª?gˆbàßÎ!?n¥+»]O#?¬bÅ4ï?Œáðo2M?íEÌ8ëð?¡âPˆ	ú?¢·\ü†ú®?"8Š¨3Ãñ?¨ëß{zFd?š$Ý]w¿«?îe¸Cû¶ü?Ÿ¢#"Dòý?N契"´?Z¡PˆÎ4å?©(½.}~?Ÿq´¨§Š½3FGL J0438.8-4519@oY._ú;›ÀDåù jn3À9?ÖbwÄ]À;¾s"LS?ëÅ`ûK@^d‡éîÇ@!¥?êüŽ¿â¿®{¿äpqÎ_°%¿è
žªÁ¿æÀVò!'nAGNbll?î;\ë`fÃ?¦ë¹
%ï?œpúéØP?™ @#r9ó?œñ™	O_?Æï#ª?í0Q0
?±ìøI¡A?—QäæX'ï?™ÙÓнè¯?±b<鍕?¬©c|òª?íYÎ엓f? ~ž_¢4=?¡ÌðÚà?'%Õʺ,£?¨–!#uî¼?"vÄ{•åÇ?éç¢LH¢'?´ÎÿËT?°ôÍçÉö?£FLü®
?¿Î ‰Ó!€?±Ôr8i«3FGL J0439.6-3159@m"†_•'ÍÀDZ{Q^—À:fùû@ýÀ;ÆõPy•¿ùh80)1@ÅB' Ôa?üT}?ñ²Š¿ïý¨é²z€?ïýÎ'üÚm¿éDúöÄå?ÆÁOòlÕ§AGNbcu?ïí<@Ëç´?b¶€!¡?H_Æàý5Ç?R8×û'?YWš÷±ÿ?^râG ?ïÇÉ:B.O?yS(UïÐê?GgO¯'v?M²Å&‰'á?y95ôòæ?w,eq	?é[óÇ?ŒAñfq?€_ÊÍï?öOʆ9?œ¯t¶¹K?"$Qo—?ïçã?{ùG?süÂÀ†!j?'êT4?@>IáW«?fž'1uG?sÏ"Awµ3FGL J0439.9-1859@k(¿;ê'ÀB $€	À9Õ~ŽÑ¿À;ª7Pþ¿õ'óžá@f' 'ìÚ?þµá)¦¿çÀØˑA¿á>š'LËá¿Ú¨—Êr»›¿Ý¸7´¢3œAGNbcu?ïù=ê¶#M?IBÅ¥Nžó?%Óu¨Ü÷?œ¤S4Ú?Hcš¸½²Ã?H'š€	|?ïÀ:ýD‹?{m»ÇÇ?IQnM¸Ú?QGŠèaü?|¸S"|ß?yó0˜Œ?ïkŒo¾á(?}äA(­TÝ?vMÁԀ˜T?jžÿÓÿ¨?‰ö&i²?w¨ê³'þ×?ï¬t[EŽ?{ô0È?>÷æPâuvè?ÌÜ·A\™?"Öö+>à?{é¥&Ò¬ñ3FGL J0440.3-2500@lT2TçÀCÿ·äÀ:ԕ(ñÑÀ;í(åÒWP?êìãZON>@yAôl#?û–×6&-¿ïþ~ôãÓ`?ïþÒúb¿²@gÏ2f¿éölš:²AGNbll?ïρ;a?¡¸0C¿õ?"ˆ œm¡?ž~ï*4Ç?'ûÞ&̀?‡ª³±?áv¼UÜ?Ñ6Å/Ë>Š?Ðz'9©{Ó?Í}Ã]pð?É
#=»°ã?Âüê'X™?ë=ޔ+?¬±<µ´êg?µSÓ¼Õ¹:?¥"áyg_?°ÃӔ5¥u?"¨2ZÕR?é¸Âmù`?Áp!̀ù?ÃÔRi0hË?Á\σè)?¥"{¨[š?¦œw×Ñåó3FGL J0440.3+1444@fåw'þLÀ4zƒ?»òÀ9WIáËa"À;Ip:$¾ü?â
!÷N@]E€gÄ@(k 7™¿àh•ž?ú¿æn¦ü®'οèºçC_j
¿á ¢Ç둉AGNbcu?êJÐYR|?À»†xC1Ã?´'2N½ÑØ?µ'³ŽÃu‹?¹'JéšM?µÈ½˜>ßü?íÅ	%N?¶ò¬Ú?—Œ'&"?¡»žÎ¥j?¨)ìeçÑ?°!'sÎ/?ê´~ËàÆ?ªFËR'ÐÌ?®'–-¨?š§	J›"?»>"c?¢üöÃ#,ì?æYURP=?±"ªO©Û"?ª%yßbÅ
?££HZoj0?Ц¹oå?°¸ïöl'¢3FGL J0440.8+2751@e'@¿ã°À(h> Ìÿ"À9È£¥¦îÀ;oW6Gºª¿Í
à6i§@2ƒÄ›%
?ÿ0/}HÖ¿Þ^ëì*h½¿é
M`äyð¿Å³Ï¿Š2ã¿á±¾™XV-AGNbll?ïâué%ÇC?oiT÷í?.D™œßk«?.N''»õ?k¥Í@jÆø?n…'w¢{½?ïŒñ+®z?Œ'‡¯Éï?`Ïðu+h,?b¯½É×Dr?ˆ¹ɇ‹?Š!ðYa4?îÁ"‰pé?{â.‰	­?…£\ÀfQ†?v'd¬©%6?
|~º+?‡'}zÒ¬ã?î-G5¿×?›ê3c?7oC)?AÁÝY"´á?¬ü®—-öB?›	N֙äj3FGL J0442.6-0017@h¦€Ÿb0wÀ<vŽ ¿"(À7±åvø…À;EŒ^G³ô?çÒ4oý@»O)@÷Íÿ§Ày¿äê/ô^'¿çÜ+0ý›¿æÃÔ;è¿ë›‹¤•¡AGNfsrq?ïåÚWZ?c98.ÿÇ?[þ˜'ËÝH?[c³;?XMG)€?V™ÛPa›?ïÅ 8÷?y¥Õ®F?Ov¡òޙ~?W-û§èé^?y"¥(Ÿ=?v‡Xɋè
?î*÷DŽù?šÍB¹¬÷Á?—üÎLƒÙp?ŽFÓIünÚ?¡RanK?"Èבm@Ç?ïçÐß~*§?rðºÔ>oJ?'‹Ÿî´?¤§'•ó?gÍ_¦ÚÚ?ráá?@63FGL J0444.5+3425@dþÊ€àÀyU E…EÀ9æoD[y£À;O®²0?à3-;Cð<@¦|«ø@wÈ_ÂX¿ Ôrªä¼û¿áýò?¼È¿åQeà7@¿ê½ZÅÑäAGNbcu?çŪÛe´Ø?ÃÅúühòì?Å_‰1g?Â󦛃?·– .r?²ˆôÅmih?êƒ q;g<?ÂÃ]¯mc	?v® 5q¬?ŸÂ>/{É(?ÂD¨w´Ý?À_MÊ1Ø?èåm"[ß#?°ž§ˆOO³?Á‡TIÛ ?¨Ã[W¯"G?µÅëKO©? ê
wÆT=?é ¦šPjë?ªúéÌbV3?¤¹¼ñ±¢?'ÄnètÆ?ÆNöZ~'ë?§«lÿ!±Ï3FGL J0444.6-6012@pàŒ€AÀCs`ûH
À:\f('ðÀ;ïë‹Ô´ù¿òaohی@^©WQËz?ÿ™¾×ü¿î#ߜ]?Áh%£8æ¿à•€œêÔA¿Ö7‹~ñ*AGNfsrq?ïø覚o¼?IMaaúÂ?#a†ö?#w.ÏnJ?G…$_'Õ?F×
ôúî?ï¾ÖùYX*?y'²EÁ4t?Ji–qåÄ?PQ¶øÎf?}Qv …®‡?w˜ÄF›­Æ?ï°¼ÊÑG?….Á³yÇ?¡{–N&?o×;Ò?"*››0?Š/eµ%m?ï׹ɢª?pŸðñ"¾?çi`Ý?$z&ï?s«}‰}–è?p‹·|"v3FGL J0447.8-2119@kŽ± ‹ü"ÀB!ÕߛªÀ:Q˜y*À;ÉlËu±?ÄhÔÏ>…æ@GrÄm­­@`¡ ¤$ã¿äY@í ¿ç֗4u¹§¿åÍ‹gb÷¿ïÿ{j£ýAGNfsrq?ïm"ñõX?ŸÑõá¦J?ReTYé†?QXÚ«t?›Ký|{¶h?ŸPŒJ¬)?ìè鬔ï©?²g…ùÞV=?šÃ\Õ[™?›©˜\í?²ÛfÀ—?¬E:L^?H?í-ùøÀ›?žPÆÉ&=®?¢Iƒy؇?‹"-î¤ð?ªÖêæ›oA?–÷é±åŠT?ê"6ӝÐ8?­º;'ð}Z?¨ª·vª¾?ž!²;¡ró?¿ˆí§¼0?©º{ªf?3FGL J0448.6-1632@jà»ÿŠ;ÀA6¿Ý/ñÀ9AÞíwÀ;\ä
[2V¿àÉ`í¼Â¥@'_?ý¶¤^ïy ¿ÅÜpGª¿Ýˆ_ãý4¿Õ»Ö[åÚ¿àXU¨9UÈAGNbll?ïês(bé7?f"Äa?;½þá·?:ÌLC¯0°?b,?Ý:'È?djiLKÐ?ï¨zû%#?€M œfN?SéL¡vð¶?WàÁ?ƒd¥GÙN?}UmN?îÍ?#wº?3 (À?ŒÔ{x¬´1?|ÄaÍ~"?—íÝÔ±NŽ?"ìQ³ƒ‰?îiˆ»¼?"¡J(º?;øP×ވ?>þЬBŠ?©1d㬄"?"AÒ#'q3FGL J0449.0+1121@gm ìt2À4ª_ºz»À7䨮àR¼À;:ŠE–ã?ý€qÅ?9Ò@¾‡d¸¼@¼³Ž7eÈ¿âFWÔ8 ¿éU;)]Ê¿è[•'ïx–¿êÙèögêAGNfsrq?å!ôÅ?÷¢ýl‹?"0l-З¯?šDh7?e´j&Èݹ?eØTí¯&y?ï^1•"?›¿Dð ?tНll˜?"r÷A5©?ôdäe7€?''e>Ì>w?í¥]°¬{?¤Õ9›Ñ"?¯è÷mÆñ?¡Èç|õ»Ø?œ¹en\Žy?'ï"h8ò¶?îK4mWá?©EÝ-'ô?…ÇOú÷þ?‡îzöcš?¦šå+Ãë?¨-l6nŸ3FGL J0449.4-4350@oΠwmÀCôäàõÀ6Ñd‰"—À:Léki¦?åÅ~Ä¢@Á]Z¤k?ý•\ ¿Ó•¿ÜFž†#¬>¿Ýs䧯޿؉k?$iR¿Ü+ƒÆAGNbll?ì'f\Eî?¹†éÏ«?PÄÔ¾ð"?cÓ¼{^?»)¹Ê؄%?¹MlæÉýT?ï¶)'}Ҏ?¤ÀÛpþš?I¬Fë£Ð×?P²µ¨Øµó?€Ú×1ÑŸ?€Å¿­¸X?è@ǶÑZ
?³6w;	ˆ.?•ÏÐn?‰?
1Xwï?ÌBçò¦£?²¹÷?ï?ìÀ©—£>6?¬eZ–f?8é{î?CP"ÒÏ¡?¹â¢BÐ$×?¬	H~/3FGL J0453.2-2808@l¡i@5z5ÀB'HàC¢À8iüybÂmÀ;ŸüJhÙÞ?ôPBàÐ9ê@ÓÇ©¢PL@
€€mùƒ¿å`tԊ¨²¿èýhæÉM;¿éf¢®7­¹¿ìá£ÙŽ|/AGNfsrq?ïå…6[m?l/‹¥L?\êØìÏrü?ažmþa?X
»y²S?cˆMŠŒ™á?ïIÀhÍ"È?"ÆD…—)?lJ%lTIñ?rC‡xƒXW?">®8Ñ£?¼ 7Pß~?î3<ÿ'l…?˜ÙÊ9´¾O?¡iC"¢@?'©àô\\ì?–ÅÙmï:?P³¿Öã´?Î,ø>?¢ðO[TÁ?…dá'Åî²?'"b0~½?Ÿµq~Ü?¡èA_­(÷3FGL J0453.2+6321@bNO€Ü3r@(Y?µ!µÀ9v(ßóÀ;[‡æï?âEi™KÀô@'–E&@Æj?Žá/¿ç¨8_å:N¿ç⪬]ãØ¿Þ²~UNÅ¿ÛÀŠ0'flAGNbcu?ï¸DêNð?‹9‰œeé?QVV(ºØŸ?U&i3XÂR?‡õNÏR?ŠKÕÔsã?ï2q´&C?£+ÅTvu?sî6Ã&Ð0?u>sl¾?š¾$±ƒ®?¡kŸ©CíÏ?îߎTåQ?"s]ÑZíê?~Luk\õß?s­ôX=õX?œ{ Œx?'c™l¡Ùy?îôr£Êˆ?Ž·žX¤€E?`—%˜lù™?cxH¨H`?Ÿ^ÆÓ¡`[?°ó˜v3FGL J0454.6-6825@qzw@=ݱÀAÚÁÀ)P[À9óLŸÀ;ª>"E]?욆 \p2@ðÑ›¯ô@"ä %\¿ãƒ"^ϙ¿äJRŸ	E#¿âB;¿┿ïÿ¸èz0OTHERpwn?턬±‡;?¶ƒ^A°×?Ÿ¸>t[?¦ÖÙw:¹^?¨2wÈR:?±@fÌÖTÏ?Õ²Ö¡ëυ?ÇC:"Š"Ï?ۓßž÷²?ÉÈ(#än8?Ír"†êq•?¿ïqbû4?çvMú1Y¶?³°Ša[ŸÅ?Å4q$ÞcÄ?®äžÃñ{ñ?¹ä­ä¸jÊ?¢"¶«|S?Ú9;õ³?¼Pq6'?×°W9©5Œ?Ágâ‹qÄ?Ìn߄5©ƒ?³e|Z-3›3FGL J0455.7-4617@o¼@ŽÉÀCi·?œÎÀ8Ÿ>õÀ;¡1$e:?ï.9Ķ˜@ßqBn=@^àAHË¿å^WµYÏ»¿èBs'‹ò׿çw'&Ç¿é¢AcÖßAGNfsrq?ïñ«Ê~¼ú?Wêy»?BdAQ_ӛ?;­³tŽ^c?SvJYÖ$;?U3PCë›?ï5ûj'°?'µÃYßó?qYÃ@ïj~?t®%‹XÊ?"ê!Ýn#?H×úÍ?îç²ÝdŠ?‹_¦º*L?ˆUÆ?zYOÐÍ?–ÈùÑâÚj?…Ù1\°ZY?î%ç7¸¬g?§%›j	ã­?‡6c;t¹?ƒ|["h?§Óó¼¦\_?¥ª»éúˆ3FGL J0456.3+2702@eì&?šIÃÀ$ÔHµ{À8෋òçêÀ;-hÁŠyk?ñYžqŕ @Q¸Ð¢@®i t)¿àʵ4D¿èAÐ…h¿åP‹¿¼C¿ì8ÒXõ1AGNbcu?îå¼±¦Ç?žŒ\Çur€?†¼'[×?‡½ôØô?˜BàÁxó?—"RgÈá?éG1ú?ÈzT­ã}N?£-w	¦[?¤:©±7¯{?Æë…øö®??Å/w
3?ì¿<k0þ?¦ºv(ïá?¯äµŸ5½)?›æ:©G°?¯ßVš2ó?œB8_â‰?éÑãE4ä?­4"ýŠ2G?¤=\4h_?˜äm¦"â?éÞ¼?¬€Â¾Må"3FGL J0456.3-3131@m+VŸIÀB½¿é{À9ΈJ¼½À;æHEéï?áX쒇N
@㹯c°T@MbÀi'¿ã
ºægÊâ¿ç©¿ê;Gª¿è1Nˆ	Š¿ïÿãï—ìµAGNfsrq?ïøM@ÇШ?OzqÕØ£?`Ê:æ?#¸ÜSVZ?Jþã™z<Õ?MtÇ:¿n?îßZtf"?šÖÒ':-™?zó½
–?}¤_Ä­?WÂ.8Y•?–[*‡…¹€?ï)'Ïvk?'Q²|—#Ç?ˆy"7‹ê?sì0?8Á?&u‡êÙp?z—yD.òm?îà)5?¡s'à@­?'ùÃ̐Ñ?Šn™ç‹{?¥1`/ä\?žO+3FGL J0457.0-2324@kö©Ÿ¡—ÀAr–¿Ê…ËÀ6uQ'ÑÀ:£º¤¬S@–íw'2È@ Ïryð@à"@¿7ä¿ÞÎmЁҿäQÍ_™Ã‹¿å–À™¿éxŽûAGNFSRQ?ï(Ã7•h?™Ä<¯æì?xGÜ!ã\m?€ÞÌ]4?"Õ¢ä;Ü?—gö}â»?ïŜn¯×¿?yðe"t÷]?J'-žCó?U5›¶Ã8µ?yߢôK¾V?wL…6¸5?è ¯¨­|?²EӐØã?»r1«HE{?§¼E`—î?¿°×rN§?«#À%¶?ïòŒí!—s?mm=ˆ{ð]>ð–ô·ÏÕé?9ss?Z£Ééñ׋?mb:Út·½3FGL J0457.0+0643@hDàÚ ËÀ5°cÀ™¸£À9ämBùyÔÀ;r#QA;¿ÿzr·Ø@ÎÆQ@a:ÿZh¬¿é ?Ðû[¿ãu&ǃÑu¿ìù×bä¿¶õÅÿÔ0AGNfsrq?ïº/4ç3?"º§\"V¡?r¼Nê5?{™©ñ¸å[?pÔ¢1"?x%‰–yOÍ?ïÊÖû	n?wçî-éÎ2?N]Ÿòž?TƒH)Fs?w%à¡ýr?u¹ºÌ´õý?înÈZgÂí?"=">Ño?'Ÿ†Ü0g?ƒ8Eǟ"6? C¶ëu8ø?˜°i%C+?ïƈ4̾?vxäZ§>ðåMKˆø?	ä±3m‡?|«L†n
?vwl¼ß=3FGL J0500.3+5237@ctÙ_í¦a@e©ÿî7VÀ9h ƒ-FŠÀ;]€
|ZÄ¿Ó`…'F§ë@
[¿Pã@Ë àJX¿âæ=@¿ëD8>4îõ¿Ýa'Èýµ¿Ø—ÁREG2OTHERspp?ìœG	ì?º.ú¤mÙí?uËßÕÁÌþ?w>íVb?¹Á	b£"×?¹Ñ—Ísi?íß¾Ž%Ø;?µäh«×?}m«7gä?†µïØD¡
?®Va¶µ½?´oOb©íY?셹şr†?¥>JbéH?œv>Í$ðä?‰4Ð^3s–?´´¢»/˜?¡øvpÓ?íUfû? Ë¯SOp?_7!áÏòJ?`×؜Gæ?·J³e͈_? Âã3|ê3FGL J0501.2-0157@i.
á'6À9E  œWºÀ81dÒèoÁÀ;Zl ºŠ«?óÿ2ªøÈ@³¬wâÆ@OB?ë}g¿ã÷|k¿ä¿æ@àùˆ¿å¥\jÓ¿éñ•S0KAGNfsrq?ïîÿ¤Ã,Ô?VbÜAÖ?P⍤ZF?O¸Ä.Ø'?Q(ÕLL?Jhbg7?ï¿ôñ{€:?|o|XÂ)?Tb!ºgmÁ?^\Uzò?zìþÓ¦%?xŽTÎïžÞ?îèz"gäí?ŒSTÀWµ?Žõ•Ü}\?"ì×UË?"æ²È#Ó?"ø\²Ô0M?ïÍ^®x_'?}ØþI®?60ÕëI\'?I?²AÁÌø?wí›e¢U?}žÈä3FGL J0501.8+3046@e¤(?NÊhÀ5pÿÇuöÀ9Íøí½]À;WQ§'€¡¿ÈW%«¶&Ã@ÃɃl0«@þÿÝp^¿Öfm†¯ö¿éíq—
â̿췋aiô³?æÉǓkÆçAGNbcu?ï=CxÄn?›ÖAùŠ?z(æ§
l?')딶zÉ?'ÍWx]¯Ì?˜2ܨ?îŠX°ÀÎ?¶Óñ,üÉù?rïæ䎊d?‡j´£Âòµ?¤ü(b!æ?µ?—ßY?í3ö8³/"?ŸÇ•?¡d@a:ô?'•®ò¬}?«\\/Òæ?•‰ýéò_-?ï€Lë?•ÁŸÇõ—?¼å ½z?.Ìå»±?ÁJ‰ÞG?•¾™q¼ÞÒ3FGL J0502.5+0612@h>ìß&k¥À4Ó>¿XpÀ9ƒÂl º‹À;'ÅPÉ?¬î"É€[@µž´5§,@¥¹ß_K•¿áS¯¸пì4k‹>b¿áÁÄ|àë¿ïúÕ	öè™AGNfsrq?ì;ü«¥!Y?º®	—A;'?†,;à‹?'¸,wJ(?»LuZãÒ?¹3ÅߢÐÔ?îö )V?®Æ2ù?'®·Suén?'Ý dr»?¦y:UÂuô?¨í¸•Þ?èçæ£zZ?®k4"Ÿ"?¶XÝ¥Xi? ¼	­+Ç?Á3ö¡d?§ÐK¦r?äý¢ŠW*?¶ÚC璁?›ú‹OÇß?"Öå@n'&?ÔE7Óº?¶ä6ç3FGL J0502.7+3438@eD¼@ŽÉÀ:ƒ?»òÀ93u@ô¼ÖÀ;=KË°m?ìN–ž×@èÆUå9Ö@JL`€É>¿áÿVÛ6¥Œ¿àKTš¿'¿è:¼¢ï>ù¿äû¹*>ÔAGNbcu?ï£ô l
?ZHÀI?yÛÈތžÝ?yJô:уo?t ==[t?q¾C",PÔ?ê"g-mÈ?Ȝ§W¬bÀ?'ÆŽ0¡"~?š{˜¾êÒÞ?Ãy'6O?Ɵ=(Tc?íz:Ù(?š1V[6ÙZ? €ô{B?_5k¨S6?¦xF]óY8?'ÔñðŠ"?ïÒ^§-d?'Ä"=Ø3c?d™ÿÁÎÍ?hó4e[Ñ?™'t2àÙ?'!b°×eù3FGL J0503.4+4522@d7  ôØ@¯rú6<À98‹ò)ôÀ;3>iȶ?jÐì1»@˹ÕÁ@á€.¹|¿ÚÁFíá¿íqÑcµ\¿¹õ¯ÞÄ4è¿áO.+AGNbcu?ïÒéÚÍ`?|QÇ_˜vk?2ÿL;a‰c?4ÒhEÌQ?u[Õ»·Â?{«ÂÃ?ã«¢C•[¶?ÔÕ¥¶\z.?Èâÿûœ‹?—)Ó?gÚ®?׺t`Õk¯?ÔUcT4?ìx÷رJ?¦Ê+Ì>?µlfQÊ?"'–«P?¸3ä0á>?¥Üé#ä?îE×7MNv?dW.,?3Ú均e??ƒ7ÎuG?«zØa_ݺ?U3Râ¦3FGL J0503.5+6538@b'Î ‰ãC@,Ñeaƒ¨—À:X4õ«hÀ;ÇPܑeî?Äà5Á¿å@.ûJ¹@®h@0FÅ¿éqÏÔÐ7¢¿Úü›Ö׿ì[
'ÁË?Ù£@'ªAGNbll?ïjk8=¥®?•©e"å?…ZJã‡÷ ?'÷v¸?€
ç
Z?ƒ›ÆÀ"ü?	«l?"%æ'Fy%?f¶ý'ru?q»³}œ?‡ìþ0ž¢é?'eq¾ž?î>õT㑈?"ËÇMâ¤?™"bµl!?¶í~ll§?Ÿ ÂØbê?Šó‡›N?ﲏoI_Ë?"Nž]ï	F?M­ßOϤ?e)ÄhßÖ?So³[?ƒKEF;/3FGL J0505.3+0459@ho0_®¼AÀ4ÜW?öÀ86ÈqyŽÀ:ô÷eýŠÛ?ûaܶ#é@ób–x'@Ïï=*¿á½Ë"Ú¿æ@*†!¨Ø¿éT‰;Ÿá¿è?nO"æýAGNfsrq?ï̄Gù?r¥sõ€P?\iÃÝÅ,È?avÑƺ%?r£k€8*?p*é?l"¯?ᆱ]xþ??¡/S"¾?UíT!"}ô?\pÕ-¾¹?{.ü;Á??{í)§zÚ?îuìút"?ž1F­(z?˜ÌNé¤á?'K² %?¡¢y»†­<?•þ@‹?ï¼tÆB?ƒµrrÛ¾m?3lŒQ³?HB[d?€`¯j§f?ƒ"ÅJÇ
3FGL J0505.3-0422@iŠsÿ¬*À9…Üßi‡ƒÀ9Лx–ê"À;pæDm[?ó[
/')@
֕Î]ñx@
ú`-è¿ÚeÙµàÄs¿ä˾mA*¿çÏé°Äi¸¿ê™¸õˆAGNfsrq?·¦¹ñ5?µv!¯±Ås?áç6T;|£?ÍæZ:Ç?ÖGäÛBì?ÍKØû±?ã)ÝFjÁn?É?ÇÉ÷ŠÙ?Í2œµÉº?Ã]ŸO-"Û?Æ%îߟ0Š?¹¾6çöÿ?Ü»¢,Ý?µ5XÑz©È?×C /ÍÖ?µF,¬
?ȅW{HD›?ªøo×¥^?Õüë?·&•'Ò–?׉wQ£'?À›H\¶Á?ÒzqÃEAJ?¶Gþ¥ºüÁ3FGL J0505.5+0416@h…Ÿj"óÀ54"Ÿ^ÕxÀ9Џº–iÀ;vVO—íÈ?ÒG»_ç5@<OM:?þ}q +Y?ÝÕ«:"]¿Ñõ¿èÁS¿¦FöLпäHMÌ#1AGNbll?îù¸'#Z?Ÿmf(Ø?zLÃß¡ùu?"4¦ÍΌ3?š5˃3g?šèƒLÑ# ?î8÷Í>‹?­ˆ¬
?'CÊ Éh ?"úZ˜Ç>?£]2ÇcP?¦±äÓî?íÊa1ӈ?˜É!šWh?•ë¹Ü"!ï?ƒ¿ÿÍZ"
?¨dô…f/?"x¸%_¬Û?êXu ÁFX?²NÜ.˜d_?g§SI5?›Ð'-¡?đ4''²ø?²7Ÿ+JjÛ3FGL J0505.5-1558@k&€IRÀ>uàè@À:7œÓ	ý°À;͵±þm¿àšŽX•9Û@
2"¤Åœ­@ÐúÀP»¿×'ƒk7¿ábvs5¿ç •—‰ýx¿Ð[±e¬ñÕAGNbcu?îýÑ틨õ?¢rOh—ø?x®rit?€‡;߀b?š@qðœè?¡—Õ°'ëœ?ï—mñ?Jo¶è:s?^qŃ,E?d_ü@4bV?†aÏ6º?Œ·Â®¹?íªÑqµñZ?œ3bë4ô? e
Z·§^?'ÁvõØDõ?¤íމéBð?™Oÿ+p?îé6¬×«Ý?"!5l´Ô?Q³Íf*£ø?XŒÀqS¸? ÞöÇSí?"{o_¹Å3FGL J0505.9+6114@b¢¸¾øγ@(0¶â—À:òÿf}À; ºö
´¿ñçêc5¯@(
e‰œ¡@;À n ?ìŠb=(¿é¬l'zk¿¸'eŠzº¿å5¯CéAGNbll?ï¦Z.¢ùý?ÚÌIàV±?9rƟ".?@i¦á‡Šd?…Þ"HoB?¥—ä®?lW;?°lŸgôƒ‰?ràÑÓE´?|KšÑ›M?¥yT§ #›?®•ýXÛAh?î'Á-óO·?——'rÜ ?"]gsRš?u#Mà©?¢ÎUÆî/Ø?•JýKÉù?ï¿@^Ñ?" %Hæf?"kâà"D?17à×S#)?œCAÎ`"?"˜ý'¢Œ93FGL J0506.9-5435@pf¸À>-ÀBbë@UZ¥À9n?"zM¤À;P9Ø?çÅ
uÀf@ð»"k1?ù¥Ã P­m¿î[þ÷tô§?ÇÁXXg?²W\PT¿ØÞR—bÄAGNbcu?ï©h r—c?ƒ	ué±Ó§?U‰Ó¥¾»'?`¡dG'ä$?'ô½n¢OÚ?Åh¢6ÉT?ïM£,ag?ò<$ؘH?j™«@â¨t?mÛéã8¬r?'øe¯þ"?Š}O¬Ø?í¿­;ž¶l?™r<Œðƒ?—Œ^j~?‡­BûÊmC?¨DfßRg?"I›³
&B?ít/úÀ?®û¨0§+?x´é"F…Ã?'†g_hž?µ™mKÁ®?®÷ì)Õòø3FGL J0507.1-6102@pæ}ÀTïFÀBtߥíeÀ8ä(í_ŒÀ;ª3Ž¢Å'¿nyJè³=@ü^h–'@%ҟʋ)¿ç¬DScv¿¿åý '®¿çøbí¥¿éø^i¨÷AAGNfsrq?ïö5Ôĉ?N>­‹"¤?;ß.+''þ?:Ìàٟ(Ä?I<a—ZG·?G¶'‹ Ê?ï­/?'ó×·4¿d?R»ë{k·ð?XœX<:mW?'\ž‰Lˆ'?H0Ú®?ïù
=o?‹	bÜM"¶?†ëYžÑ®¬?}Íëÿ{€?"k1èéGÁ?ƒiwûÀ®²?ÔV¦?‡À`ý''?HHH_¹7?K!
Ü7S8?ŠÌI5Ða?‡B\+ð3FGL J0508.0+6736@aùÖ`^åi@/È)?"j†À8CÕAæÀ:¿Œž"#¿Ï'Ÿã	Ð@lŠQýù–?ø]q?ˆV%¿¡âe+ÓÿἋw¤¿¿ÃlJÎQÕ¿ É^¶ÍAGNbll?ï9èV>B?¦KŒ?49ÈÓÁU+?<P€*.¡q?˜rè¶ú?¥óbaê?ïŸ}ÿjK»?"c&²m.?a¥êEÇ?eÄxl)â!?ƒØ–ÞòÂ?'u•î˜±ß?ìB»öÌ?¨ÕB1¼Ó?•ò9*Ü÷M?'%ðòtç÷?ºCgŸiÌ?¦
ZoÛb¾?î"ÙH›g{?™œ®
1P?"²÷Ò?4Ê+×ÏG?¦·!Hp?™Ž*"a3FGL J0508.2-1936@kŽ(`ܹªÀ?0Üà@GÀ:o4bÞªÀ;ð).ˆª?éK×V5
J@Uµ(Á?P@ÿ^@}¸?ÔdQ^þyS¿áòÆ7‡¿åGQ¯Z¿ïÿf`˜W`AGNbcu?ìÊ<Zª€n?µ<vcÛô?¶zs˜Š6\?´¬ýºG"?‰L'1?‡Åñ'¾>?æäÔÏ@"?Æ8bKiká?Ãf °oÏY?½ʞòY¢?Ä:KüS.Y?¹ƒc\fga?é;½«n÷Ö?­@Nȓ8Ü?Áã¯n'i—?¨£À³Ý?²Z³È9n!?›FS_Ës?ä͆*TÒ?ºÄË\©Ë?ξ€5[ä?µÇ4ú3…?¼Î@]'<?«7Xz©ýá3FGL J0509.3+1012@gëý`éNäÀ1?Ê ¢¢WÀ9"Çë¼|À;Vj3z€Ð¿µÐF¦"C@#ȶ@zÎ]=s¿çÂR6ôe¿ç?lkQ÷¿æ3–òí•<¿æÎ8˜ÞïËAGNfsrq?ï駁S§Õ?e‰ì6"E°?P¾øb/?RËÈöoöE?[òSN&¼?` OÁ"Ã]?ïW(Ñ)˜?™ñÞ²Pc¦?rEñü+Gç?Èe…@?‰i[Ôzò?•³d¥©?î¢2°ZJÈ?"¥'*eàg?ŒI؋d°?4ÉDBߋ?¹pô"?Ž3 "lÕÞ?íP0nôì?ŸíӆOº"?r‡9ú?nï
"u?´Vè¿H'?ŸObsNB3FGL J0509.4+0541@hlë têŽÀ3 ¼€NnùÀ7YˆêíÀ:¬ß06)?תŠm+Òl@70BèÞ@Kù€_
ý¿Ü%<`¿š¿â¶‹AèÜ¿ÜNŠê ½¿â-ZfÜ`œAGNbll?ïֈb>£Š?x&—C"?0jðk[(?8šF
É.?sµÙøˆ	?wÇ¢1?ï½×†4?';Nyx·°?Zgn
?w"¬alOî?zz™¹^w/?ziû´ÜCt?íHðý®œ·?¥77>aÆ$?…ØŽ¡Üˆ‡?
4ª(Æ?²ýf>O‰2?£ØƒQ>ó¼?ïCSt¢»?".Å·š¶?Ÿ%±Å O?(bÊÑÃ?—yÿ¹ã¶?")ïRŽéÕ3FGL J0509.7-0400@iæàé´À8gÀÌäJÀ: È{.tˆÀ;«'Ýãu†¿¼á'Ô'¬@
Æà#Á¦?úaäa\?å6y8Ñ¿à$«œ3ð¿–Ä`X™¿´žD—<OÅAGNbll?ïé\'_H+?iJÒì6Y?,&$KÉDï?4:yä½aj?dá[ûA4?i.,þ?ï¨&§Âtk?‡P«iAüÒ?]!(µ>!?i3çI‹ m?'R0ø»"Ù?ƒÙCœyÓ©?îǝ¼ÞŒe?‡ë"W_?Œ u'SÉã?|­0ÙÍm?˜ü
›"Ž+?(¥F…¨?î=ò9"¶y? ¸.0¿ˆ?Fº¥§=F?\YÆW3ñŸ?«ÅñÐ&›w? ¦¿$Ž\[3FGL J0509.7-6418@q$·@=ݱÀAš†@ €À: s,G‡À;ä"i·S¿¿Ú4ç
ï$ï@§E¥¦˜0@wœ'"¿éêþí¿ä¦¡H:¿â\:$áXB?µú''JVAGNbcu?ïëµÕÚf?bŠ2^¤?(8"?'g2`F¡?bÇuyüh¦?a•©üXì‡?ï½?DU?¥Äi~—p?LéêªM¥8?UÞÛ­?}Õ£% â?€‰î…??ïA®õà
?hÊ[Ø@?{5²Ç¼5$?hQ'3¥
?ü´'?{Òµ–ìñ
?ïÄÏì,›«?xö#@%?د~'?!]sÿ2â
?}`XŠµü»?wø¾â|`x3FGL J0510.0+1802@gû¿"ÿ&À)‡LàƒböÀ8ÀÂã>ÿÀ;7&ùz«?åMƒ2©v@øîÀ½të@F§ msK¿ä¿Ÿ±Fð'¿åîç²è[Z¿ál;ò–ØA¿ë—6Ã5ŸIAGNfsrq?︴ãH¾é?ûL8#<?cBR×Çj"?cüZô±7?zdï¼ÖD?}å—GöR?ïQA ´1?™!ŒŸRx?tî†Àt"õ?{ùÖ&?¢v+ÌT¸?"^Ëê-"?îQ¿)b?"Ô#Jгb?—¶èà
À??ˆÌ¬m÷?ž#zÐS'?ŠS|.'Äã?í-ú1Ÿ'(?¢rˆå: ?€3|ÜÆA?vîÛ²xWÃ?´‰¾ïÝù?¡ô8yÐýÈ3FGL J0512.2+2918@eõW´Àx=`2Å¥À9®§â1¸àÀ;9WÒNìÍ¿Ûb1ÍF^"@{——᳏@@¿ ¿â@^xõùÜ¿ã2»!1[ ¿ë"j2xοå~¶0u‹AGNbcu?îÿönO/? =ꬖ,Z?‹ŽX«`BÊ?™ Ý/†ú?'X"Ü…øÑ?—*é9Æ?ì¬B4´_6?¾ý¡¾_êy?‡nR¢3?™(gb_+?·°,пì?ºö]Oúk?í±;°§Ao?š'˜d©|?˜DgÌÅû?ˆ±Û(м?¨Ê)bš?"ð'dΩº?ííÑÝ÷~?ž¨œ9ÁŽ\?f'L£T´8?i[=eK°?¯¹½VRÓ}?ü¾¨'3FGL J0512.9+4038@dѾÀ//˜?íJ =?ÚÀ9Œ$ôÀ;[a8)<9?è6âGæÒ@"WJê‰÷@͋?cÿäz±|íÄó¿ÖÔ»Ðóo¿âX[œ'¿ãäâ^É'ëAGNbcu?î)áýnfì?²¢éQ?‡'õ"¯yå?ŠÉr®{¢¿?§—âàm²µ?±4:9-Â?¼|³>5?ÇuÐa?ª¾øÂf?®
ÐtØÇî?êĕ˜È²S?ÉŠXˆÕ?ì'/åz—U?¡y"£^Ád? [_÷ð²"?Ž>¤ŸùÚ?³@ÐØ2ì?œ;"HôU?ëq÷{X5•?¦`ð_͚? K;ø¬ˆ?"ÕI,‹ä
?¼J¦žÁý?¢Ê^xÿg,3FGL J0514.4+5603@cBß72œ@$»ÁÎjÀ9|5Om&À;}Q›Ô}¿ë¼T2öç@œ,µj°x@·Ñ?Î!6¿è¡ø‹žþ¿éŸã*cÇ¿æƒxÒÇ-¿ãxÓ~ LšAGNfsrq	?ïÚّQŸ?¢mR	Òf?A`Œ+Ë¢?EËB n?pg%Ò–í?¢ná¶ÂÀ?ôZÝ@?«WãôÔã?t·®Þ´óí?zݬ+êœO?¥=ÚÞ{}?©›L-þS?î`!•u6r?˜Ú®Û2ì?"ͬѳ¤?{1r»âAw?¤Ê{t?Ò°?–?'ž
¬@?ï
|Fö°?(ëíõ?Dk3ÀK@\?Eñf£yÔ?ž
 ~Ð?Q&7Æt—3FGL J0515.3-4557@ow•@%NÀA¶ó=<¡À:(»ìª¸¦À;›ÕÎÔ
¿©åD²Ÿj@/ÑËdAô@p@.ï,¿éÝ"®Y¿Ö×c©ž¿ç±"£ï×σ3ÒAGNfsrq?ëõЕ5Uì?»®û»Á,Ó?µº¼Èq¤M?¶®TUÙ·?¥-}ÇXÊ?­+œø/'?í¦U¥?¯ÀSc䟢?•Xbg®Ý[?žñ.÷A™?ªó
l6þ?¥¤5.6?é‡^Ïôf?¬ßT•7?N?ÀýPs›?©_Cø•?±Éîßy‰–?™Íp‡Kï?ê|+ìY?®5qåWá?¯¯LiŽßú?¦E`ä*?¼Fúhpg°?¥È¹Œ²3FGL J0515.5-0123@iY,Ÿ/ېÀ5Þó_ތéÀ:™`sÞ.À;¸õ½†ß?èkÅd½^@
ch/>\?üÆ`Ìôe?Ôq'ð$b,?æ5ÓL rš¿ÐÙí­Ô¿äy¼*øÉAGNbcu?ïtÌZ5?˜cüÃÅí??n'»e¾?qЂ@tpÓ?‹XÞ&™h?–â€6	¼?éôÖþXd?•ó(n?¸Ô#¼o»w?¹b<ò"úI?·…$PËÙo?´£Ö`oK?îcQöz?œ»µÁ"	?""{6‰?†Ý?iÍô	?¤pNMESÁ?•<¡™Lº?艝8Ñë?ºàϗ]Ò?ÄóÙ¨™\3?¸Ápt c?±Ëbî¸E?©½û#äcÚ3FGL J0515.8+1526@gwÿ´€¦À*"ÚA)•ûÀ8Ϋäõ¸~À;.Àp÷Í¿ò±ÞÇ;@$M˜ö\@ŒÐ¿u¡B¿â׳Í2´¿ãtsè/(â¿àèÑÝz;¿Ùø1<ìxAGNbll?ïŽW|C?‡tRHÈ~U?NGo²ÿè?Nó'/j'o?Š•³?µ¿C?†ÄdÐoB?ï°Ë×I?ˆÈE$\½?XŠDÀìŠï?[ÒD»«Š?€»ñæ,œp?‡œ|¹%¶î?íe_NRÕp? ÄXœˆØ?–žsH1™Å?‡gouLÙñ?®ZÑv¹Ü5?›'®W?î­ÙU<¢U?•íjÜÔX,?#ð(Zùñ?0\ðV[7Í?¥zƒ¥¶?•æThû
3FGL J0516.3+7351@aSÊ€à@3Æ"à՘MÀ9ò¯ÑêBÿÀ;ÐùyÔt?òá']
9@‹³÷ñt?ÿu«€vÝØ¿åM¤éXôŽ¿èôA¸Sm¿ÍgrÓº°H¿ÖÊBÐpUAGNbll?ïh¶ÓT*¡?—<(庲?kËQ4^Ù?t(絏z?Žß"V¨@?•_½8?ïwúÈ4Â9?'ÈELÞ9?{'ý"x¦?Ú5
:}Æ?"8Opµ]?Šú ¤Ë?ë«;Zén?©ÑXö¶É?±4ñB™³? ‰ùƒmt?±r
9ÎÙ? f•æÿJ?î°Kà?žŒ!JÉø?y{¦'?ˆÏT[Õ?¡Ø=Ïî-#?š&}ª>2Ã3FGL J0516.7-6207@pø6ÀP½ˆÀAaG P À8/›fù3]À;JbýüÁ?åãÁ¦(U@pyà@)Á'°—¿ÛN{Òοãhxt…ãÚ¿à–€Ï7$¿æ]º,§ÜAGNbll?ïìf9¥¶]?`?(Ô&?(Î0œZ'¼?%¼÷•OŽ?bãPƒù"?`-kí ^Ù?ïr‡<V?¢÷Æ@'r?cK9÷"0?gf¼;ñÙ?Ž‹jó!ôB?Ši#çüFc? Œ.Ð?—EáOš¼?ƒ™ðDܸÚ?uÜiÒwÃ?¡?YæäÇ?•P\m›¼'?îŽ
eO?¢D'Òi?i9äŽÑ?h»:a\ÞG?¬×v¾ ?¢\½íÃ3FGL J0517.4+4540@d^\FR@÷QÿÒÊÀ9ËzdJ,tÀ;UÂ%©Ý´¿ä>ÏôEÑ@hú?v¸@°IÀheo¿ç²¥4M¿è¢9`ýN}¿àî«ÌÌ÷À¿è3MU%ÿÍAGNfsrq?ïï\n)"?a]R†% ?2hŸÝÈ?rž]‰e?_ÔçTÞ(?a"@R:U`?îr¬ãG
í?±]ñŸŸ*?fì£ùÕê?r¹Œ©Ž'Ñ?§fg‹ñò‰?°åÈÒÌ`V?î*ØÉEó?"€9åāä?ƒ"õ.æ4?vŎُ´`?¢4²vç9?'GãÁqÅU?ïÚÊY躴?o]ž%ù*>ï`2t=>÷ÊñÎRã
?r‹#‰à?oK­é¸å¢3FGL J0517.5+0902@h0à?pXXÀ0)ÃÀ´–À9Æb‹æR°À:ùŽ,~
¿ä¤¤Ù$R@Ë°…ni@b»q"î?黎W4ÍÆ¿ìñ÷MB·¿Û­ðÂåC¿áä|í͉œAGNfsrq?æ÷¨lW-$?ϬL³"1?h&¿ó«¢?r6.w€Æ¢?Ñà~ÙѾa?ϓ¤äÚÅ?ï'ÆÍÇÖc?'4ø@sb?d©ìE*µ}?l@Å;Bý?†cÑ|¿¹Ù?O4Pâ;%?æ4DÃnx?¹ãm*X9?¨cáLóz?˜V&Ï¥ù?ЊúO"¯o?¹õ‰¯ôÿ?æ›JT3?½ô¥Öš	é?RvÊcÉ&?QØ¥mS?Ò¶ô6Ó?½ìÿY•èU3FGL J0519.2-4542@ooý¿HÌÀA]›ÿ¥g-À:QÈI°MÀ;qÕÉːÀ^+¸ën@R#½Iw@ááÀ¤ËQ¿ãMsjƃ¿è;ԓ¯cŸ¿êÛ¿Z½¶¿Ð²­3KÔ6AGNrdg?ïë¼£/x?ae¾µÎ]Û?Fãgnå^ð?PVzieM>?]éF‡?[^¥D_??ïʏ—±æ¹?x‡–WaË?G¨ÝÏÉ?¥?T9P9@½?wÃm{"?v²ù«Š+?îvOER{?'mUÇ,UG?Ž¡Ó_ìÚ?€ž²¦:"? ò–ÎÿԘ?ŠL ëÑ?ïԁÐ
½+?uŠÌ;Ž>¹ïr50›">Ô§\tž7?u½y~J?u‰AH±á3FGL J0519.3+2746@f:" ³Ô®Àá'_Á0·À9Ó[&—C~À;iï‡â¸¿ôËó @݅6‹,n@¤y¿^¥'¿ìS«lfð¿âö:qÆ}¿ÙÝWu9¿â~'ùZAGNbcu?íÃ`ï?³5>®(Ý/?€/V©É?Š½õà@?¯£¾-x¤Ú?±ºéY©ØD?î8܆…ß?°yhÀâ?{,ñ¸C?‹'O˜¢"?©" ™"?¬!ÔUÿHÕ?ë"þTü/?§ßÝ0î?¡ÎÙ[û·?+ĔHƒ'?ºp¢§Z''?¤Zó·YD?í%[>ï]?©ºk`X'x?18]Ùv
g?2Tïëó9Ý?·%œÈ/?©³a¢»3FGL J0519.5+0852@h=쿱[WÀ/°¾|§ñÀ99{*BÉ©À;šþô?ùÀZ*ÃÍö@'´#lÂ?ÿﴀ¥¬Í¿Üû¾Ê"¿æWdØi/'¿è?ÀDb¿ïÿ¾ú¤™AGNbcu?Çɛ BA'?¿m¿Óò?ÒXÏ­Ñ.?Éïô­‹¨?àá1Aë"?Ìs÷sx­¿?ÌÿIš½dð?Äò?¾5az?âÕ§#{?ǟŒÕç~?ʕaò¦
&?¿P}?Ѷ̐%‰s?¯÷fze×?Ü°å+ìµ?³êßïñ?Ò*'Š®‰Ù?±Ø/Æ
‡ô?Â×â̵?©õ«õh.1?à9!ñ"z?ÀEƒ"=?ֆP+ΐ±?»Å.ú®w3FGL J0521.4-1740@kuNóÀ;•sà¢l§À9ÇquŽ!–À;Áó™À0¿ø›«–ò@ÓtMéÄ@nó€jÉx¿âBå'Ñ++¿çѪÒ'¿çi ÙŸŠ¿Üç¶vãÐäAGNfsrq?ï	Ng,†€?¢ôéJ0?pšBºÂß?tÓEù†ã­?š²Ì‰À`?¡ÅxWƒˆ?ï¸cúüŽï?€l)xš?T… }»:€?ZiDØþàŽ?~¬ºbI¹Í?|ü¹g2?íÊäüÖd?œ
à|[qc?"X®I1%ç?'
Û6³‡b?©šú‹šÊ?–qÜþ<áµ?ïtÌôìL×?Š×qѽÙ?!o)ÿÛß0?.*ŠyGëS?'Cƒv­C?ŠÅ:tD3FGL J0521.7+0103@i)rÿÑÜ×À3T‡`±ñÀ:5:¯(wÀ;š#;nk?ÏœÓ+¼@pÁFóµ?û-€H9Ö?îâw]•Ä¿Ó"¨)Ãf—	'›â¿ÇEnbøâAGNbcu?ïú÷ÄʂT??¹(ÄÄx>?'šszâ̼?'Fž"v׎?<tŸî{ùý?: Ž)ff?ï°ºPh·?"–Êž?\@Hw¤ß?bíÿáÕ>*?€sÈ\ñ6r?'\t͍½`?ï¬[á~w?†ÏN˜gÇ?ƒ[9%×,M?t¸÷hò§£?'|×ðäšò?'7ÄS^?ïLvªQ?¥XUÅï?<폯}†?OÞ!šJßX?–Zèì·á?p‡I3FGL J0521.7+2113@fó'àÀ!gž´JÀ7LªÓ}ÁÀ:l²oStò?Æp^'ê@ëH>³?þĤ_E_Ü¿ÜÙ©Þ¿à
õò"Žp¿Û°Š¡Ú¿ÜSóÉAGNbll?ïKÖQõ_?œeųy?/ÖpUñhŽ?5ˆ(Ý-?–EˆþuqH?›úJ914¦?ïCö¯ÄZ? «ûæ'Œ?cU{††Ù?p"gX"æ?•Ž96™ƒ?ž{÷Ÿ
?éÙdn'Ìä?¯ª¾Q™ýô?"BNa?"-÷×Jª?ƨ}~§‹?®•#K%?îâk™k?–=ØF:&?FEjÜÍ?#–Íaµõ?¡Í,íƙ%?–<N€âJ3FGL J0521.9-3847@ni>_·¼À@­? (ÿÔÀ:?³~G-¼À;Ç?QN§-À¬âF[®ý@^VYS†@… êÚ¿í=ÌÍ´ºn¿áƨR⌿äì~9R`¿à".¾¯SAGNbcu?ïþÁ¹Ün?&ÙÝUX0>ýÜî Â1ñ>ýú–;m*±? (Äuá?%fT;X<?ïÍ&ç÷9?yHbPÂr?FcÚ{ìl?PÊ`^lN?v ï¡fU?vËYü7ŽP?ïR÷ÓAáY?"ä¹?yÉÅËñ@?oNs_Ôá™?Ž]{L¡°í?Nþô‹ê?ïúÌ*wó@?Fõý mq>©©Ûœ0>®õ"[¶O?DÍ@ê÷Œ;?Fó'óX&Ó3FGL J0522.9-3628@nð`»+»À@[ò¿¥œÝÀ7ë×TLÀ;$†îœ*n?ðZYŠµÑ@æÑZÑ@/hDq¿â§ÝÖº}¿ç8Á5¦\¿ç%]Àƒ¿ä}óKoG¿AGNBCU?ïî™uê?\–Áçõ]?Mõ¢ßì¯?NAÓ"oÆ?SÓaÓ%?V=ŸÊ€¿?ïÆÂd­v?x¶FŒ¥ä?KÜ·ÑúDŽ?UñT§rcª?y#6Äéì
?uœízԆ?î"-òD¶D?–%"ßg×?'%íQ{Ϭ?‰Š¤Èæ?žTTeíh?Æ[ÂB‹?ïØôÜîl?{>¾ª7?†,*©õ÷?¬˜9à¼e?sCxØUu?{zµÖ·	o3FGL J0525.3-4558@o}Øÿu–…À@Ùr 0ŒÀ:VHø"À;Ù®&ïX?âÁ©\t	@Ñc	/ª@œôBp¿åØ ¬¿â	õH…Ä"¿×suéOY¿í€±b°qAGNfsrq?î"¹hŒÜ?¨ûË0Ê1D?™³§ŠÄU?—ö‹Ú_͙? ú›…?¢Ö‰Ìásœ?îìYûZÁ?¤í9Ðê3?ŽÌ jIÓ,?õé¾d–?§NE·ß? nFÍæd¶?ê†õó:ñ?¬)9¸œG?¸‰—¼H%?£Zï]GoÅ?³>¸©àw? $_	×h?í
Iܕð*?¥R›n Û)?"Ññi5U'? ¶AÝ´/?²y4Á)J?¡îÂIWší3FGL J0525.6-6013@pÑ̀CRÀ@ïÇÿÞrÀ9•üÁ‡mÀ;zšéû±½?ñμI¢á@EpOô4?ûžŒÀmBù¿Òæëˆ
X¿Ü2Ýð-¿"œb2
zi¿áD‰8ð®ÌAGNbcu?ï¤"ì?"˜fm&"?mòÊÍ\î§?lÃʦƒÂY?~õ‹Ó.?€JRï"Öå?ï^íÌw_"?úl)0r?l/LÒU|F?pÏîóÛ:a?œ\ÖÉ^?xŸ…àT-?ë›õ\—[?©z\Å¿?±¥îó£? Ž•®Ú?±zf' Ö? .'ØëÇ?íSçQãj?¦ÊiVîj?uÎü{Õ¨?€ØoLÁvõ?´äcÉ'Y?¥à±pPüE3FGL J0525.8-2014@kÙq`•l
À;ñ Á¬À:[ìSzÑWÀ;ß:ZMS?–PnU_È@zû¸G¯—@€V@(¿×®éö0üÖ¿á¹u«dš¿×ˆ€º¿èü·•FèaAGNbcu?ïÔùs™?u†^ãè
'?Z8Z}{?]|4ä3©Š?nعK§p?q'cÉ·?ïR—nΘ?'oßB§&x?p»$®<Í?oô-ÏÐu?'~Hú•ð?6'3)â?îtÁ|kâc?•Ý°!?–IÓ–Ck?Œ`Kyú?›Nžíp2?ˆÏ®ÿO?î±/+u8?"7ÃP±+d?f«Yji†¨?c:ƜJÜÍ?£'W²ô?'˜Áoßê3FGL J0526.0+4253@dÔ_õI@Ã×Àâ¯À9\sв4›À;SÕ™êø?òmJ(B>i@óa4Î=æ@{ðà}XÆ¿Ùm¹,˜­¿êzôE•¿åÌ
ÏmÞL¿ïÿàL¨ÇAGNbcu?ák?·4˜,?Èb3áüúm?ͼ
W-:?´Ïë'Wž?̖öÌ?ÅIÙùN­¨?Æ;¼ºŒf?ÄjΩڼ?Õ˾˜;pE?ÅC•Ò?ßc^gIˆ?É)Ҟf…?á!ò—Í͌?¶2lÊÎK?ÒÉÈÖ<?²CŽÊr²Æ?Åæ©Y?§Ò›êÃvï?Õ-v>¶‰?²dðáKK?ُJ4ƍ?¹a—6¢àa?ÑC?¾û=ê?²X—6!ÌL3FGL J0526.2-4829@oßU>öµÔÀ@àn¿Ñ;ÇÀ8Êû¡ÌnÀ;\¾óÆ5Ú?Ó¼0ýMô@N˜|äG@NR@i§Ž¿âÓ»Ôàu)¿ãÏ¡t?©¿ã"¢3ž¿ç…l1g½:AGNfsrq?ïØDEnàâ?p™'7¢¯&?;!ÐÁҞ‡?5mCšãë?r+À<rd¦?p$ŸäŽ?ï¿ÀüM•
?{=;"(›n?Lyí{4p?RÚÐ=T?|_†Ä?xsmáFc?îсñB?‹£Ô±âÀ:?†‹wI#?w¤TP€3?šŠ6'×—æ?"ˆW^ÀÝl?ïßkíx?ÚRV4û?.¤d¡?1{
Ñ?ˆ
¨Œ€u?€õ¬Ë–]³3FGL J0526.6-6825e@qm~KZÀ@lӀE4½À6_MkÝyÀ:?æW¸Mº?þOI"H¢@èVÁèb@u°Ÿoœ¿ß¾Nî÷ð¿ã7we'+¿å³ß@¿äÂôÁÞ\AOTHERGAL?ͽ¤f/o0?‡ž3§,?ÀMö÷?À¢c‡÷Ë?ä}U¨¶@3?Èf‡
hVI?ÄÌd¬v.Ð?È}$KHâ?ã²¼©`6?Ð'·Éæw?Ìh¨¯lPT?ÄÊW½àY?ÓR~
"¥?±Èœ{0®'?Ì̚׉"?±-]ܾü?ÞG4‡'ú˜?´1\AÊÁ?£‹)éH?ŸèlAÈö?ÛU6UÑR?žD¥"Û?á²DåÿC?Äíah¦ˆ=3FGL J0526.6+6321@b"™Ÿä6v@.†þ "ofÀ9úÈ×'šÀ;͔ãQs?è
™"GÊç@hfʺMï@Q·fw®¿æâ?j¤
¼¿ãTR+Š·¿ìJªó€&¿ïÿҁWèAGNbcu?íQù`'Ã?²Ä'0îLî?²ëd-$<?°"_Ž"$´?Šê`FŒí-?˜h3Þ$ÃF?âp6ÊÜ?ǀª{=×?Ò!oÀ
	?ÂñÿóŽ¹e?¼ET{§?¾ué)CêŠ?ìŸ2‡~í?£DZ
¸]?°&½C«[R?›SÎ<Œ\ÿ?¥¿]ºp`?"¬9oã¯?Ý¥@<"±?»£kT=Œû?Ýš÷XÈ?¿Zf,§¦F?µL"0f?¦ëQwi.3FGL J0528.3+1815@g^·`¿]yÀ"d²—À:s'7ËHhÀ;™;ÞÓ_Ž?æ5P÷¿>Å@qZRÜÆÀ?úU{?Œ?¢eÉæñ勵¿7¿8Sr]¿ÚäP¨u:Ñ¿Æ¡eÑýŠAGNbcu?ïªÀgŒô?"tt½Ê$?[¯Ë|ÔkŸ?\ײH†‹E?ÙìȂ5N?'´"öÖØ?ì¤ÕpàZå?¿Êƒœ¾?ˆ-M¤é0=?'uÚ à;?·ÓªÄ`Ì?¼½‹©œD•?î.'ࣺ?˜GDhØ!?"ì­2. Ñ?"Ëþ"€B?£'¶èÞ´?'8pUK7'?íÛÃ^Lj? ¾Y-¨Wù?³Tä'0?ŠàIç]çS?­Öôâ5ø;?ž=õ6€3FGL J0529.1+0933@hSvÿ:Þ"À*è¬A<
rÀ9fµ¨ÃÙÀ;DBì䚿æ
·­Å@^&ˆó@ˆÏ`zê¿á[Æi¿çœÏ2å[¿ìY "Qº?×0sêwFwAGNbcu?勇C΢?ˆ±C åB?w·2͕œ?ƒµ3ô§?sÆrƒè?vÂ˹Ãóˆ?ï¼ó'ñÃ?Š³_àòu?UÆ_µ_š\?^Ç_z‡:¾?|§/8'?‰JôªYÙ¸?îÚ!W¿?–³ÔÝLO°?–­úv6Qa?‡³œ²?¤›`³¯[q?…<©Iâ?ï"Â}ZFB?‹Îµ?ù8=?F±]-ÚÏ?§§›p1?Š¸øA]?‹ÎêjÐï–3FGL J0529.2-5917@p¿j€JÀ@½i@5z5À:\(^ÃÚ¶À;Ú`S&ÛSR¦¿@
—>•¼ë-@ÿÜ TsË¿èüî8ég¿åuk—RÂp¿á\6°§cm¿ØSrÇ^AGNbll?ïQêQ?™W‰KÆø?Mv"?‡Š?JCi˜$ä?"ä(`¹§®?˜ø­,ºŸ?ï =Šs…?ƒŽøÓ¿µ?V#|úÿV?Zہ¤ìŸ?… xóš~É?±{3Õ½'?î<"üŠkÃ?•ï‰ŽŒš]?O°fn°l?xû-KZ¬<?¤éä½—¬?'oYKOÕý?ï3P2ÑY?‰ù'$å?A(•Ã"ƒ?FÿéŽQý ?™´÷¸» ?ˆôµkúm*3FGL J0529.8-7242@q¼¿šÏúÀ?×ÇÀ'áÀ9«èYM‰À;ªÔ}›6¿úhßè]vÿ@/€3;@ÌπsÝ¿æ^ï_Úí¿ë€ [ՓƿԬ0ÈÓK ¿èü2•ÿ[AGNbcu?ïý\SÂÜ?4(\kù¹>ìyEÍf>í]Côs‹?4;€wÀŠ?3ÄɟÂã?ïÆ£žÅ;ç?y«´­Í"?MSûfŠ?VZ'ÓTÄ?y±<•;†?v–8é™ù
?ï:v[-p®?"B¡VCC
?qo¿ØÃ#?b-Fˆð8?"UD¤-¹h?'覆‰ã?ïÜᪿM?ptžã:c>ÕvýòÓ¶>åÛʽ­Pd?q‰Íûw?pqO·_dÄ3FGL J0530.8+1330@gëü–þµÀ&‹$£MÀ7ºÇªÀ;ÒÎn|?ýËk[BÆÏ@._@B-¡ú¿âúžrœU¿ç—Áf«õV¿èêPⲊ¿í'H¶ÁâRAGNFSRQ?íAãÛLŠV?¸VHÌǺ?°à°D`^&?¶×*Ŗ°Ñ?"@Äí<œ?•Œx:|?ï{Ð1µ?–	þˆÐ'Ç?i©á¿H¨?r²ñ¢Ñ€?Š¡‡¶ƒÀ@?'Þ"æq$õ?ì¹Ò"?¨˜ÎA"
Â?µ
Ö?£ØÝrÃ÷?¥*j@À´H?—´'ÜE®F?îÛð—dË?¡ñªš¦?zN•c£5‰?†§_—s_?îGº"Ù? 4˜}–á…3FGL J0532.0-4827@oà 6mÀ@g`#VFÀ7F™¦.ÓRÀ:¤"Øi¹?ö¨Y-æ&@0¿»lR?ÿ}•øÛI¿Û¾òˆ¤¿â—:·6¬¿á;—ÇB°e¿å£^™4ç5AGNBCU?ﶅð²ª?²¡`ŠTe?:ïX
flw?@ÿÔ.:R?‡B€"9?ߎö¼}?ïÏ®þV˜?u'P6¬?Fɔ<v·?S'¬è±I?uON1Åð™?rS–"¯Ô*?íerÜøj?¢Þ4VrF?"Rˆ–yÚ?Šàåæñ£?¯ÿ'¶óŒd? šq\ñ?ïõ×ÃÇÍ?bLKoŸÞU>ÖЕ[Ó·?TU‰Ñpÿ?T9§Û
á?bF:Íù3FGL J0532.7+0732@h›5'Ì÷À+sóþiýËÀ7|äJ7\À:ޖstkã?øVV"÷@ʖpÅ:@¶¤¨ÁTÊ¿á^jL¶"M¿å°?é$h¿ä3Rè°-/¿è6¦¼þàAGNFSRQ?ïÀÇ%Ö=?xǸ"?U'ëAS³Œ?VTcãa…ç?z;²MßôB?wåøªÛn?eT_:?'•2ÆW?UԙÔÑ'?a.ËHW?{È/[.ªÇ?€&ԑD@?î[`9'¦Ñ?œ»ÐX¦Û4?W¹È¶š?"òJ!j?¢ô
ô§ìv?–†
nv"L?ïÀlŸtQù?'ûH}'Pa?$ù‰w÷¶k?4º	®—Ÿf?!ãúEí?'×»-:p×3FGL J0533.0-3939@n˜¬B»fÀ?d;ߪ#À9îRŠçO/À;¾ê·™^áÀš®ý®í@A
;|Ù@æ½ÿ|¿×¦¾laÓ¿èØKIeµÎ¿æ*EEPäk¿á_"½'"AGNbcu?ïçÉ*Æ©¸?jŒ|.Úíh?OÞb.¶Í?XëL½~ûe?`?N ʘb?e%©¦"e?ïËÈ´½Ê­?vÛä-?IòJ}rN?P¶wǁ€Ô?vëgWÊû?sï;ð¶?îpÆè?ž?'ÁFi†d?'ÞÕÅíB?…é@zëGï?ŸM2ýRu?ˆ8¯""
ì?ïËßKFÒl?vÛ&Å)_}>åÝ@œsÍ>ö-ðجIm?zk¼H°?v×Oöèl
3FGL J0533.2+4822@dE$û¨'@ rE AYÀ8uŸÕôÀ;<ERðgÝ?ë¨UTxÛ½@f»ŠPG@__áçç¿âå¬H·˜¢¿å±'ì>hW¿å•™(ýǎ¿çn[b¹fAGNfsrq?ï۔A±?l-öR#?SÉ'pÔ?QÎ7"'?jßí:?gÜ	yž?îåª:%«?¤"ëTo?mœ<Sášï?uÿ©ôB—6?Ÿ—10Îi¾?£ÍGpbÿ?îm¶=ª^ß?—d¯Ø?m–ÀŠw?'"9—Å…?¡É6¤)ïq?"Y-«rz²?ïuïýR˜?2ùâ?TŠr9m&?[ â{@kt?ò¾Žä+æ?Ž×U2¨úZ3FGL J0533.6-8323@r|˜`fÀ=&7PþÀ9Xå™LlÀÀ;š¬±¤RZ¿Ë,Ž@'á@æ±÷ßJ(@^*€J¿Øcî‡1¸	¿å\"åX<‹¿çåD¤Ž"¿Ó†fŸNí×AGNfsrq?ï÷øïw?Ky'ª?6ô·è‹™?6ÓyΤû?D¡æ/ØìS?F]6d‹>?ïÄÒM+­?y5nÈëg?MÒbŽÀ?VJhÍÜM?yܙF©W1?ve­oÁe?îéñ'9ý?‹™&8ÚK?Œ0µˆÇ"?'T›Gþ'º?"©s{àP?€×ÎäðÝr?ïßÔÉÁ'k?n ס+0>üÀs ƒ?	&Kp"Ú?oñµ?–S…?nà"3FGL J0534.0+6759@bÄupÅ@22g  ‰xÀ9_UÅ.rÚÀ;¾ÜÛ7ɛ?ù¿y'3J°@`ñz¬¢?þµðØÜö¿ãY©Ìíƒü¿ÖºØª6Ûð¿àEåÝÙ©¿ë}™–ȦPSRPSR?Áö,aJ?»VÝX_%?êÿ4Š¯ö?½n
+×,œ?hõGÖö?'l'~FÒÒ?ÚJꙌÂÿ?Ëx"@a?Þːwê?Êٚ| Ô}?»§çWðÔZ?¸Յå·?ÐURûQõÞ?³º§8Jæî?åp¾áQ¸Æ?µ³Ô¤ŠÔ?³$½*bV?œr—*?àÛ|žŒ²µ?½˜Å[>ÖÖ?Ùz¤˜ÄÏM?½šúÈܬ›?³9ˆ¨‡-(?¦vuYmɼ3FGL J0534.5+2201s@g´ßݵÀö@8ªAÀ7®X¡UPÀ9×U,'?
?êy@wƒ3@dN>a@Ý_Ù.…¿ïÿô!O…ú?ïÒj WS¿Ùeށ*7¿ïø¢©Ô$OTHERPWN?ÚECø%?ÒvÄKs8â?ác(p§à ?ÒÆÏêíº
?§£Y5€Í0?³J¦ñ<?é`ôõô?Õ[jfS?ÂV¾—Eo?Ó[Þ¾Bá?²§{)ŀÔ?óòÕL å?Þnú†bþÜ?³Hüõä ?̹X´±?®Â⃿š?Ӑ(ÍBøË?²;ì‡S?ê!Mgl}?Ñ6¨G¸JÃ?¾&Óó° °?̧'@ •_?°ÎÀÐëvv?Åú´h­2ƒ3FGL J0534.5+2201@g¨`ܹªÀ_?«'"À4V8/v~À9D›	Ü!Ô@‹u>›q@»7»ƒ#a@§FÀÙ¤w¿àï÷…nP¿ä'ÛÇ¿å5Ò$O•"¿êÆB9`sÞPSRPSR?Üe´æÂÐ?НÕîè'd?Ôe°ˆiu:?ѕ
'±;ä?Îi6ã_ê?·c(*N?èdü•½?Ññ+Yý@|?¬•ÿ"g?À<Å/æ?Çd†C‹îœ?ÍN'☳?ÕSÑÒ¶¬¤?¹"]rûñ?ÍU*¹Å·?´¡«ìb¹?ܘнð?¾÷N´TŒÜ?ÐÈB͆?ÈT˜×Õ#?¸Uf%
6?Ã5<•Hä?䙔L7w—?Ìà–©Ù3FGL J0535.6-2749@lö²ßP]À;ëÃà•®À:oGÆ;À;ÇjM{³Ö¿æ®S+z)@
"½Y'B@Qç_u0"¿ê=:þèÜ¿æóh±´¿äÏ\wWØã¿ÖàüFYxAGNbcu?ï¬hPí@?ˆÉ-»Ñ	¾?Q"Çll\?S}dÆçà?'Á©W!ì?‡¨5âÒ$?ï©qñÇøÚ?‡\a%÷‹?];(±‰~?pÆ֍V?[?ü¨ë˜w?Kk/?î"ÁL¦Wï?"C'u‡Í·?†6°d@'?z¶Çº?¥ÏÝh`·?ÐzwÓÇ?ïcפ‰?"¨+žö-Â?0fɧ¢?5sA©?"BÍÓ¹=­?"ŒrFš3FGL J0537.4-5717@p˜Ô_õIÀ@6ä?°8À:q6Ô¨À;Ûµ_Ƚt?×35/s2@#)@oòä¼®¿ï¬qó''?å+ ¿þˆ1¿Ùé+(]þI¿ß#Ú½GÁAGNbll?ïù÷˜6?GG˜[þªu?,yсóó²?/ÃT
þ½?Dͯ•")&?BLÂjØ?ïaÌnÐ,?kÜd.šG?gó{B`^É?rcRîØ°?È½°. ?ÕCOOå?ïFÇðbÇ¿?…‡»ÅÐk?}Qù(²9?t&/îˆþ¡?¥RôÐ?–GýªÃ‹?ïYPК?^škXr?\P>
?{mÄBu <?Š õ±Z7?Š=ŸŸàòµ3FGL J0538.4-3909@nŽ@îÙÀ>E`IôÀ:SÞKzQÖÀ;Þ|WisaÀf©!¡æD@¹'ùïÔ@S–‡å<¿é	ܘġ¿Õc)%úKÇ¿àðº¤ùk‰¿Ý1*Ê®å[AGNbcu?ïú`~*Äô?U¥àQœß?!Ë«d',Ž? ‰5¹&´©?B{˧P?TÙ·\h¸?ïÎmڌ%ú?v~aÁð®Ž?JPF¡ ?Q$rfwñ?u	åÊÀ?t*ÏÜ7?ïYòðàá?{²%½¶·.?}6}J9?oÃ7h€t?Šõ(¾"»×?r_"Ì˸?ïíÛènm,?bf½û†>κ°yÆ	!>ßþ†•[èÌ?bhåta¢?aÿ/+Žr3FGL J0538.8-4405@oB¨àÉÙÓÀ??Ï"èÀ5æZ¬ôÀ1À:Œáû2;?ùŸu‹ÈJ²@§9Bú?ÿ!L{ƒ®÷¿Û°.fçZ¿áÍ.õk¿á\"ÔvËu¿ã>oAGNBLL?íLõ¢Ãö¨?¶ÇB´j‰s?Fû­8Öý?QT©ÉÌA?µl*ò…Ù?¶®c:œõ¥?ïÆÊ<Ô?x£%–é:?HÖ¯͚y?Qê؇~f•?y€@Y?u÷7Ðxk;?æá!b¿³?³»P'Çå?¤ä
¿‡S?—y&,?ÏBy",l?²e½í"ë;?ïáiYw‹ê?y65Á¿u>áê"YËέ?ó'2:†?n"¼I·?y1b"}ç´3FGL J0539.8+1434@gófŸê%À!B™`
Ü·À9Wßh°Ã'À;C2Öìá??ò8=-ÝÞÃ@Ìy³JDÈ@'(?7?Í02m¢à¿æ<¯ý»¾¿è­f}bT¿å«þ	rAGNfsrq?ïЯ'ñúb?'i–¢S`?sIPd-î?ÐØD÷ô?Q{œz"?`È£¬cz?ï,ØxŜ?¢ƒ{ê;M?eò,+;?s\óǖ?—¦¹«é…? æ»Mñ@­?ì"ܾ*?¤D©JÏÏ?§e"Rt5?•î<N~Ù/?°&Oåud?Ç벸½?ï¢"Z?ˆƒûÞdºÒ?>Ÿ'çO|?MR¶ÇªG?†…žµ:CË?ˆ1€É¤0Á3FGL J0540.0-2837@mŸä6vÀ;@>€nOiÀ8ǵƒ+ßÀ;'j&ˆ?í…9Û÷j¹@Äo~)£@:Àß®¦Ç¿æë|ݘ™¿ëÇg©m³H¿çÔr¦™:¿ä½ÁA(AGNfsrq?ïü&o>ñ¼?AV¿Ók?$ñ=œ«?&å0UD˜?4Sç:"C??Hˆ£%Õ?ï­Øaᒫ?'—ü'7?\¯œ1b.¸?b7ºo	?€óôod?Àb_<À=?îÑÄkV¯?'K£5«?ƒ"ü +%?wþÿ—Ú3?›ýg—,4z?ŽO7öˆ$¸?ïfÔõÞA˜?"íQ£¬?S"ªÁ"1?YsC¿/x?'ì(9‹´ó?'ῧ
ù¬3FGL J0540.3+2756e@f‡ÔŸ"…^¿÷þG€óšÀ7=ò¨(¨–À:"~áS?Òò"|/a©@{pkÍÙg@ŽHÀc1þ¿àÐÜ&$¿äŸ™±Ž¿ßÔ$"ï"¿ç †
 zOTHERSNR?ž—M¦7|?¡Maì=Ê?žÔð"y|?¢.ÆòD˜?îkÄö2x?¬1‡•U[×?¼ûþEÂJm?Äë…Áu=?"õUÍú$?½-¯¯ïN?ç¿BáÔ8)?ÈH-‰ÑF%?¿pI£;—?©'~òL—b?¼0­'¢©¤?¨'T˜)?è‹á8—CX?±ö±¾ÎñÌ?Ì>†úP
?¹wÂC"y?—KWq@3Û?'t}%G?è6¤wj_?ºœ}›~¢3FGL J0540.4+5823@c=éÀ"š_@,'‹ Z›À9P0uєÀ;€ÍÀÓg?øsÅ@~-'Š[¹@g  ‰x¿êoœß¹¿Ü÷&o!î4¿ÙÿhI¯:Z¿Ý}õ×KñAGNbll?ïÒgš…Iˆ?{.*b?kˆÎìaô?p¤HœüË?b'Ü«ÊÍ?rÉÑñkÐF?íœÄ¬?´SüªðÌL?—9ªfl?™…ëN•sŸ?ªp*"Ç?°pG¦ýØ ?íÃÖ9A¬?ƒ&5‡?Ÿµ[Ý2$?'WQßOg?£çðmÒã,?"€:ÉG³?ì#bŒºÁû?¨È4æ;0??®l±X??œ9ÙCÒðò?·yPmÓà\?¤ÿšÕG3FGL J0540.5-5416@p_öŸÏ=ÀÀ?ã^è¬À9%Fí$[)À;²u®ØÅÿ?èûµÈEËß@ žæµ,@ãßbüz¿æŽ‹î'¡}¿åឤJ¿ê<:áÛÛ;¿ïÿâÖEé¼AGNfsrq?ïúóý~ 5?@S‹ÑC?3äÇ/tˆ9?4¹PoK¼–?4{LۉÄË?3%r_·jg?搜TŽÊ?'g|¬Þ?WJ©±W?_øâ¼YýÁ?'•™U¦"'?€:Ú¦uè?îçQ_¥)=?ŠðßÞÀ¾a?'sMLŵÓ?'&%ö¶Å?¢†¾•"?°!#zâT?ï¢3¥íQ?†	båžï*?`) T‰Òø?d"@háV?ƒpkb7?"jò?Ã3FGL J0542.2-8737@rÅÈ _ñØÀ;Ð!`¢ØÀ:Þ$
%'À;·ª1—QÁ¿ò×øyùÁ"@LpjKM[@OÄÀ
÷¿ì|_ã{¡¿Å£/ð]¡¿Ê'Õލ¿çô%g~ÐAGNbcu?ïôåºTV?V: "f?5ãæB?1q?5°º½	É]?RO:úLJµ?S³ŽD•·o?ï¶cyÓhh?Èz*êÂ+?Xÿl‹‡`?]"(ÜÙøÀ?~Žgóióã?{Ú1`~È@?ï,pÝào?‡'ßÎÒ¼z?êZ$2¸?tß3­Žå?'ŠÄÒ*•é?ÝD8±b?ï¥[ãÐÝU?2\ý»"?$OLÉm?0
0;¥Çâ?†XµÎ•†Ç?<ӜüG3FGL J0542.5-0907c@j¬ú D®†À3j矶êÀ9'ï,»À;
I"®P
?ð…««iûœ@£">‹«ð@Š1€€˜í¿æÌî¹9P¿ævx{Ö~ì¿é_}¹
Åx¿ïýÀ~FDAGNbcu)?îbƒëìÐ?©rB;üì=?›cFŠñZï?ž?rQ¶é?˜L;÷t¡V? wÂÖ]?ç­GßѬU?Å÷2Ë	ê?Àÿ4Í;Å?½|¿¹]ÞV?ÀK«³~Iê?¹#±m%æx?èSêSÇÇ?´g¼™&.6?º	Ö@"‰º?£–'qÛ>g?Á«k¡P
?¯?aÅ?Ú؄9K­?²Ÿ‹vãÑÖ?΋>¹ˆ9?´È/Sˆ§U?ÕáÜw׎Î?³œT}ùŸ3FGL J0543.9-5531@px+àXšÌÀ?z⟜èÙÀ8œûºöásÀ;bƒ'Öß?Æ{Jï<ŽQ@õ
j?üF·2»?ê¬ï^ñ¿ÕˆÔC¨e(¿Û̓݉w¿Í´˜õ&"AGNbll?ïôy­€Ú?VzàfîÏH?$@°Šbù?%£jÐ!1?T…Ì'ìý>?UÏÙ	­—a?﷐-V1!?}ÿ+;™'E?SNÓóÞv­?Xuïڐ˜?d4WïҀ?{U|òa?îU&©—l?™Ù†"?Š˜lVºw\?'ªçåÉèx?¤zPà;c?•­ùsJş?ívspf?ª'ëP°#?TÍÖږí?\Q<{ii?·øú$z?ªXP3×ÿ3FGL J0550.6-3217@m²€ÿÚ@SÀ:'q_¾¬yÀ:?¢óµnâÀ;›ÔÓ+‹Ÿ¿ä¶Î'¾À@
ØG)_J?ùÖg?Õ-¿èJÙºñØö¿ÕÓòr›x?Â_9è?U<¿à$ÿ³ÿÌTAGNbll?ïúï†8'?@Ø|l÷?œý%ë2?4ÿ'É ?@ïþB`T??ZÃò'f?ï»ÝŒ‡Î?"@ÏO?T_š¥ŸH?Xª¡l@Ý?}	â'±?{ó;ÃL?ïRŽÔ, ?'!;W%?£#0áPÚ?wÆĉO?‹Š¹\gVß?wn"Kz?ï–þYgðP?"AgBZk`?>XŒ´ÿÏ?Zë‡!?Š.+Mw7?"?ö¬õ¶\3FGL J0553.5-2036@l8rŸYÌûÀ5¢¡€èTÀ9¤i|›\À;‹"+ÁNê?ò"žÃO£@Œåõè¤ð?ÿÃA`r†…?ïßÉá']à¿ÒW—¡Fâ¿â:.³k¿çñ'‰ÿ?AGNbcu?í½¸vä›?´<óÄ­öã?¬+ù¤aŸ?²Ü³¡|Hy?áõãµRÌ?Ž²•óhPó?ìsðx‡8?¼'~;ƒ	?§ÍZ
š¾?«€§fÄ­Á?°|cung<?³°üÊ{lX?é÷­ÙÒ?3?°¢ÁŒ"4Ý?½é"±<C?¨Ð¬fâ?²YnàÊ$? $}G[)û?çgsׁÜ?¸èýÎT»?ÂîQ÷ŒyW?±›;mv?ÀØ98?²OTEè~3FGL J0554.1+3104@fc£ –x}@cý@,À8Çy*ŽIÀ;H5Ċß@ã®:»h@…'.¼!?ú[L¬Öã&?ïã'é9P?¿ß¾W˜\¤¿è¾ÈZÕ¿ïþÊ:Ì.ÂPSRPSR?¿\I™ßÕ;?ÁfpªÈ:­?ëV¨ÙïV¶?Âð¹v9‰?—¹¾Z•ÔY?¤Ý€·2?f½!H3sÝ?'•®¡_i?éäò©‡Á?Ãÿk•âr'?È@Ö­-?Ädâ3
Ó?À†Ç}$½?¬Á
Fä+Ñ?æòoz`?µ'LÙrݪ?ñ&Äó¢Â?°þl"Ÿ?'cà볎?Š<-£l?í)ŽÔ<Ü?°ɘGC?­Ûv/Xf?¬–UìøŽ3FGL J0556.0-4353@oP`=WyÀ<®€±kGÀ9÷ªlO´sÀ;Ê/§î¿ÔaÀê–aV@'…€Þ@œ¸?wT¿Ä»Y¿±RÀ¿àšçg¿è•:í;Ø¿Ô|ÏMIx´AGNbll?ï¿Ò½¦óÕ?~5Ӊ€98?o‡Óß$ª?u®âýÄ‹?pR·<ôj?q!Ñ÷"Œ?ïµ
 QÉù?ƒÖØ\o?UT².>?VCz")/s?€­g÷;ù?'^ÆCô?îd Ýp'?"×kÌ?˜÷™¤à£?ŒOD^Ô?š"J­Ž?…b¤š%¾ù?ïcZÔ¸,+?ˆÚ<¾šd?I™OB%
?P_ƒÖ•´?'ÇÚîéRl?ˆ›®–Å[Ñ3FGL J0558.1-3838@n›Í߆ã´À:jÓ_ŽÀ9˜Q`Dä6À;–Å×Eî¿õq»v¹è@
ÞM'Ðÿ?ÿ]É^Ù)R?֋Áýïb,¿ç"	.Ia¿ÍîÉÄ&,‡¿Ú¯‰¿u»AGNbll?全WÐØ<?ŸÛÞ³@?C0E1-F³?Cäúu"z??"`e¸·h?ŸÙ?=Uß@?ï±Ì.dµý?"¶E\ûغ?Xÿ#›{š°?_Û¶"¢{é?€móc
k?'Þ'F Ç?íîÎJw/«?š¶Ý#.qÁ?'–›PÊÛ?';°æ°Æ¸?¨GÍ°'—Ç?•¯}S'«?îÂ,î'#¦?šéæ}Ò?x'öX¸?"&±"x?£Ðu
J|?šà×ÍQÛ3FGL J0558.6-7459@qáxÿûÎBÀ=‰ô?Ø]$À9´}C"À;¦üÙÚÒI?⦿aKÁÂ@A<4
Π@oß|&í?íh°HtÛ¿à2‹üU¯¿âda
~U"¿àoŸ"I<yAGNbll?ïÁ;ÁsPP?|j[Lð?b"Ÿe«"?c
гbÀ÷?vO"ցù?wyo¼t?îÛÆ"µ±Î?¦÷¶Ü[¤è?€rãËæ ?ƒÑ{2™å?œ€7cÓD?£~C¹ô?îWNî(ì?"3Iþ…Ù‹?"Ù.
ÐòÃ?…gÅõk<%? z•çì?ˆîˆ
ó?ê}ÔƁåN?´ãM•¢rÑ? B©F?˜§ž³—‰?Â\;´ä;?³žx¹ CÉ3FGL J0600.9-3943@nź@Ù$À:*Ÿd´µÀ9½
S¥™'À;zòÙ¦Ïã?É÷ù"•ø@g
}†@|­à#¿èHÛúDݳ¿ë»^säåY¿ëÖG¬*ڎ¿ïÿñY/WAGNfsrq?ïLóÛ_ûŠ?ž'h.‡A?v´'Ær"Ú?'aèYù÷Q?´z¢cí?"p^›³|w?ë{õk	?»âþÝØ6ó?¬vù¹Ü©?«B
én5y?µ@£x‰^?²¦Ç®Ï
ò?ìfqº¸?¡e	FQ?©s¼vx¢?'ÅâÂH²\?°Bu&6íð?˜Æ¾¢‡Î?ädܘ­Ù]?´lÆÏÎÞ?¾ãò±¡À?¯l¥–P?Ï]›£ïÉ­?²)Œ<Ÿ@3FGL J0601.0+3837@e§# –x}@"ÿŸÝÖ_À9ê+ùƒ=À;yóÐFÕ¿ÝÏàü7Q.@	9ùl?þ<ԟT±?²ût;Lm}¿än¯ñæ ¿ÆƄÜü£]¿àݺ¼$âAGNbll?ïQ¿pa}³?Äukúz|?Yåx]% ?ZôµÊ_ü˜?")Á<JwR?aÝv?"¶?íðøŸ5?¸Â±j@Š†?€÷7µ#)?ƒò)Ú/â?µ'Wiù?·Èm½•
A?íÕ h'ê?›%éØ/ý?'œ´ÉÞ,?¿ä(IUü?©`""ˆ»N?—Ä™o*\¿?ìÖÝ8®"#?¥2—§/¯?Vҋâ¯~?[@Ù8v$?¸ð¦ð[Ô6?¥ÑlSÓ3FGL J0601.2-7036@q­••À=Ÿ½@gÏÀ82ñc…
–À;]íCdٞ?ú#«kS51@º°Í@6ß"óŽ¿Ý-¯iBA¿æ!O$Í·%¿å0Ûrµˆ¿ç®(^P'AGNfsrq?ïìûõç©'?XHX‰,?Eöåiòó?H¸Èn·¯³?["½ø¶?Sn̕í}?ﻉ§È÷?|àѪ¥>ú?R
Yd'à¢?[394†y^?}·Ö'ŒÒ?y6àVÖZ?îáÒbHË?Ÿ}n§ÎƤ?žq%öóY?•i`4 õ?Ÿ²Ÿ¼Ã?"©cÉÀ?ïÏâÒ\j7?†ŸrÜý?,m[VIcë?9z8óØq£?w++÷™?HÏ/=ð3FGL J0602.2+5314@d~`Ï6@-,}C"À9Ñêä±À;£¾:bÒ]À©ƒæTi@«¼pP±@Du߀-¸¿í'>9²ºc¿Ã¬Ò['¿Ø ÈýµLþ¿á<$§cvAGNbcu?ïúIÍG{V?JJ^èVÝZ?+fܧeæÕ?'áÉ$°Ê??þ'prW?Fw^±V™|?ïnilMfü?¡qŒ¡V&?coÓÆCæÞ?q°ZNj"Ò?‰¯ûGb? Œ«þ?ï@û´Ç4.?†;ðҙÈ?~:ÚцA€?pÓ
Á
ƒŽ?QÒ²·éÙ?'‰¨€éa?ïÖì‰rhß?p¶÷­‹¦?]9j?Vê Ó1h?tgŒŒ¥(?pžöí93FGL J0602.8-4016@nÜ"ÿ‰;À9ó¡_`¸§À9#¾ôœõoÀ;V»ºUÑÄ?ä¾*ós«@=
¬æÓ^?þÄ6á=¿´
'½'¥½¿ÝyKyÓÍ¿Ê¿±})æ¿ã±þG÷™AGNbcu?ï'7pã?­`t¤y'8?|°Ó^1Ɂ?¬ÏÎƕç?º,®84?†5vJáÑ.?î à Î?¢:‹ÛAœz?‡Š~î,Ð?†cù*|? ^CaԐ?žyxØZnÌ?íêíAkNô?™Rm˛ûš?™pƒÔés;?‹Ycû££Ú?¤˜éþÖW.?'é–A<i?ê3õd€h"?©^"‹¬Ö9?‰æ¦¦?ˆ¨'¢Ùîž?őÀ
üÏ?©twß3FGL J0603.8+2155@g"	Å!Þ?s\žà*­À9dûy‰À:þËåF@V¿þ€v²äÄ:@ɦ$Š±@βÿœ,ò¿Ý±ÙH}"£¿åö>
3¿áª<Üv°X¿ÚõÓS'pAGNbcu?ïVž'Ó…?˜\GÃSlª?-ê¢A×?,w\tz'7?•èXc?˜Gqý(?Ð4NBϗÕ?ÔgÅ"Wò?«=e>«°?ž(TÉr®À?ç`~ón>¸?ÔgbÍfU?ëQâ¤u.?­˜ìü4T?™ŸÂåp?ÓIÝ
i?¿ú#3?ªèû~Σ³?ï؈6—'¼?pêؼ~>³o²Ä#Œ>°e0'õÏ?sº­¹?ßÚ?p铚µ}|3FGL J0604.1-4817@oö:à;>šÀ;€¦@q	XÀ:O
ª}ílÀ;¤Wèõ!€¿€‹G†¦F¬@5~ßÙïË?÷J` |!¿ï½Þÿ¦L?ïCy^]$ì?áMó½ÉÇ?˜–Œ°¹,AGNbll?ïéþèF®€?jw>Ã&?*"P9Š	ƒ?0Ó°wÂz½?d^òµ¸Ýü?ig€3œt?ïÀp·é†z?",þô¥ãh?Sä4²{h?dWT'êB?zΖ޶ã‰?'
P¿?îއq®°œ?'s•_®Î?Š;ÆR¥$D?"È&ÂT\>?—. ×Z??‰¬'AèӒ?ïÙíSš-E?}<6°à-?¹A(ÆëŸ?"|kÉtm?rÑ㰗χ?}*bÓÊÒ3FGL J0604.7-4849@pã_€™À;€¹ Gž$À:T>iƒQÀ;ÅûqûÅß?¶Pf"ÀŽ@×_´Æq@0bŸ²bh¿á7ÈK]Ìd¿í|jŽ‹•í¿~ŒË*
j'¿é܈¬ŒeAGNbcu?ïfqfª,?–Ü¡ß»~l?MO›*X?PŠ²Óma¦?'S§VR‰?–~ãKô@l?ïQ§Ç?œ¤
ƒ‹?}ÔC
r'?ƒ.háØÆc?—ˆåjœU?—°Sdªñ?íB½+Ÿ?›";¼?˜´©:@3]?"Þ"óüÀ?¯"O/œK?–¦#03ZH?íUsó¬[?©[ʅ%é?h Œo¬ÈF?ua+•¹x?´bäå6è?¨Ýkp`wô3FGL J0605.0+3756@eƪŽ:Á@ü.ŸûˆwÀ9³¤™_¸À;®yð'Î?û¾æ‡^@
|€È'Uƒ?ðü—x,6•?ïõ»tpüS¿ÔÙ3î"¼¿åª§Ç|¿ïp<"
œ(PSRPSR?cpqD›?eË¥˜Þ?ìꜺµ½¸?ÁqJ£á½?¸™Ižˆ?ÁWt
h¾Ÿ?s;"•Z?Šu¨+™>ü?ëZ蔪
?Â
Õ¥¢¦?ÁýÌ= ¬ù?ÁóÈ坬?¬€(Ê	Ê$?œ…PiIß?êumâþ>8?®­Dœy%?¾|ƒ	)/?ª?Kq-¦d?¡0«4êä?–Ãs›Ž?í?î|¡´?¬íx™Ù?ªÐm
KÅè?¦½gìXÛ3FGL J0606.4-4729@oܱßv½À:÷ûÀÖ…À:üLû[À;ƐY~÷W?Çû¿¥-1Î@Ë|½ë³m@žšÀ
F«¿ìœ­¹rc0¿¹"¢L×°<¿çöK¨ÂMå¿Úq84'q=AGNbcu?ïm½@Ù;Q?"8¼Š×h?'<PøÆÅ?Š²g"Æ_q?'T^Ðêf?†Žz¢Ä/ ?î¬Ù­Ê´?¬ŠFç†õ?":"RË×?' Bzð)? #ßZÀ
?¨/ïŽåûú?í{<[oO?›iýV&¬?S}ÖÒHN?‹ò7vô°1?©¢w>ßæì?•-ÁÅ=–?í?ÆøÃUŠ?¤~SíDèˆ?œJ¬ÂÿÑ?›ôɐÄó?­Þ:J¾é? –gÖuuª3FGL J0607.4+4739@d´xÀ>-@)ºžEÑÀ8E&s1PÀ;?uQ»´wÀ¥Ç¥EŸG@[sºÿé@.>`7ù¿äåÉkvú¿à\¬‡n/¿ßs"¦1Fc¿äª¯¶¼j)AGNbll?ï*"3÷"S?¢âä¬>Â?mÉd´Óµ/?l‹"¥ìì?–ôlêrÿ?¡ßºæ0ë?î@@£Pžo?½+5ÌJëA?zøı¡¡ø?šH¸x¢–n?¨œÝ4Áä×?¹Ê3'£þ}?í¦ë½.l?¤šŽÂÊ4?˜|8ƒJ?Œoá àÐT?±Ãé"õº ?¡cњV¿À?îö ÓW{?¡eFrÀ?7¥8«/€}?Uönø|o? f¨^¤)M? ×ÿÔ¦Û83FGL J0608.0-0835@jø€àe0À+>~ÀÐ?À8VÆ;¹²À;£NNA¬?äQ·
%‹@i°Ü+dˆ@û>_a9¿ÞÈc¬!Üt¿æêðü××m¿äŒñÍ'¿çŸ°·ìÏAGNfsrq?ïêüŠŽªí?`0L–
Þå?H¦j?Lð?Dï+¾øZÑ?^—­Š}
?[Öó²É]Ô?ﰈg©n?…RÈ3Œ™?Z ɤó?`Ž«èuã?€‰øe\p
?ƒVêÄ?î¢1XÝùY?3¨a|îÈ?‰û³y9ð?zÃ1uÊÈ?ž»û'¸·Ô?‰"H†¥Nª?ï"º8ÿÛ?'3~øºž?JkªÏ&?L"Ü"½?šî[‰‹;?'ӈÚe3FGL J0608.1-1522@kÄUŸnÅ°À0cZ _†xÀ8'™" äÀ;`l,yÏ?÷•<ÀO»Õ@O?'¡Û]@‡Xöç(¿â=³œÐæ¿ç±ë~$|¿ê±¥?s¿èKÎxژyAGNfsrq@?ïӗñrM?qÃí?©Ì?keªñä?iñD臙m?af~c›ÎM?cä'·ö¡?ïŸFàí·ý?‹"hýµ¡j?aÆ¥þu3î?dïQïHŸ?ƒ¼žDô³?ˆãÍãܧÝ?ýj¬i?"™­M ‰h?'ÐG—ä,:?‡aµB7·?šûøºÆF?Œ,ózN?ïsBT Z?˜Ã¬'9ˆ?vxGöà?{ÑþMŶ?™"…ð;?—ªy4pŠw3FGL J0609.3+2131@g£? §??íÀ &jgÀ8Ӟ÷§kêÀ:Ý12I(?ýSj-E]'@
géÝSؚ?ûè!¼é*¿àñqÇÿàå»,]¿ìK¤™'¿ëz¡5¼œËPSRpsr?Vµ*édEq?[<ƍ-5q?á¤íöP"?ÏÒMûϋá?ܟnèv\²?ÏÔÀ-/Ž?sR°mû'?'uYÉ´+?ߝìy˕?ΐ¢ž
—?àW¨èò??εp°±?±¼šò:­?Ÿr\tÕ?åܝºvö?µ`þ¯Íµ*?ϯ;žµ†Ó?³1Vöß?ŸÞž=Mu?•œ€˜9?èp:Ç2º%?¾œŠÃ݄j?ÊCA‹v˜?¼6³½ÐƒÞ3FGL J0609.4-0248@jT&Þüz:À%AŒ 4RîÀ96ÕVß	æÀ;:"Ž½ž?Ñr†]…Iß@M>A©™?þ_O€ñ­¿àWƒ@€'{¿Ý¬)AusÓ¿ÝÙ«‰þhs¿×À›
–AGNbll?ï›x»@t¿?‡ŒÙä?[1*}áþ?_ÚèÒ»aæ?…¾‹
"4?†6øÁ¢,?ïçºþá?¢\…µêi?p¹…¼è?zªKßÊu?šT¾péÒ? Sš=V­?îEŽY?"–"‹gÑ?'v9öüƒR?ƒPæMÈRŽ?¢s"œ,ô?Ž›˜*m}E?íe#!݈®?›?Ccs+‡?`wã:"¢Ë?`Îí®¾Œû?´S'×?~?šÙgò¢{Þ3FGL J0610.2-2059@lwXf€À2-ПÀ$HÀ90¾£%4À;	Ü!Ôf?óûíÖ]@q-­ã(@°}_|<g¿ày·ÜBx¿âB¨ïM¿èvN—×fs¿ìŒ»[•ÄPSRPSR?˜æ]¯ºñ?™-s+þ¢+?쌌[Ñ¥?·)zšD†8?µš&-µ"?´&A\w.?§Šq×O?¬Òõœ,Xx?éê³ß#?¾7ÃÎTpŠ?Âr"
 +?¸x%¤_dÜ?ёþ°øó?²ì6«ß¢?áLV:?´¿üƒ/RÞ?ȊÑEžß¢?ªÌÚ˜?µÕƒo§?¢gç¨J	?é~25Ñ6Ç?±j!Ù?¾8êâ^¢±?¨GþFÇ·3FGL J0610.6+1728@h" ³Ô®¿èbšë±À8ÓÿgSÌ0À:ò+ÐÂü?üEy Ó4E@Êê?«ç?þ,Mìm¿ÏnA§V¿è神ç3¿ëؒ2>¿ãl¾U¼OTHERspp?Ȗ²U‹â
?Á•öÀg–Æ?Û$µXPÝ?Ïâá~+Iý?ؐ•á¾?Í<ißÕ´?Šš$˾¶É?¦óÅ9ë-?Ȍ〟Ì6?ÄFŸso 9?ér^Œ©?Åló©?ÛîkÓdË?´®Ìµ÷ÝM?оíïá°?²wƒªñ?ÓSô<¹…?³±À&€Î°?˶‡É'Ò?»š"
¿"?Ø3¨3f&?˙LJL‰Ò?Ùñ9
ñ?ÅAL/G̐3FGL J0611.1-6100@pá´™=SÀ<O <¶jÀ9‹€ì#ªÀ;Ó\9¼º0¿þÝ3Tk<9@ˆy½0M@£Z?¼ƒ~¿é\ºO5Œ¿æ¸Á¤>}¿é`Osä0õ¿Ú•"»T7AGNfsrq?ïý»']['?1I>€ó®?![O/³=ð?!öèFòŠ?"ò:ú"²y?(Öþص?ïÈñD'?xŸ{_?).?K–­ø?P¼ƒ…UL?x#f¤:sè?vyp™"+G?ïQ˜ÒGbÝ?€®Ï÷ª''?{»þOÁà?rS`»ÈHÍ?¼nÿg?x9;{å»?ïäÂöÕK?mbÛþ‹>é8 ó&ê,>þn¡.,Ï?k$¬è7Œ¾?mX"LÇp?3FGL J0611.2+4323@e;R`õä@' ^YQ«À9Þî<³åÀ;¤ÏFúT?ÕL¯/æ)@´8V]°@Wé`}¿ë—&Z1ϱ¿ãn"±Ž"¿×'Œv4S‰¿Ø`|ˆAGNbcu?ï¢jPAu?ˆè¯#y42?Y6
 -¿?V8¾ b?¨?">ºª;œî?‡p‰£ó8?îDí†f8?´%‹vÀG²?'ênþc?‹h?¥Gƒ	?ªY¶‹Ú¤?²?£n™³?îØEìY‡?™'Úøدç?cùWHU?Xón¢Óë?¥Ð~õ¶C^?"ÿ£Êdç?î³T®ÃO}?•{¾ÈÏé?f'Blè?oÏ–䘠?£h@ìü‡:?"GýƒE*&3FGL J0611.7+2759@fõ¢Àh¡@ã:"À9«œàuöýÀ;Då1?†sðº±@.Ääv@7¹½ûN¿åÓx³£Ž™¿Ûõ>ŽŽ¬¿àÞꌃå¿îŽ'ÞQQAGNbcu?ã®6ð@î ?Å	°…F=?ÓîqF?ÄÇ%¥\é?¶Ž¹ßrÊ?²|Ý.L"¯?ê72¢(?Ã?"ꬸt?•†.¤p<?•ÌLpOº?Äsg¼éV?Â3"ø?åі5Àh?² ƒ¸å ?̞ð
óù¼?°\l^I?¸5n6˔? ëi$2Ì}?ët›U"ê?¦i]Þi?•¯MkªP?ŒV!Êvµ?¾ïQý4ö?¥7ßÎgÇ3FGL J0612.8+4122@ezWà&Eå@%Ö3À7²8%
{"À:à"Xð\?çXwýVq@@¡)3!@3å?ŠY‹¿ÙíÕǃrø¿àïr«20¿à6tJ¢¿Þ5	cÎSAGNbll?ïϹüö*<?s––¡™ç?K°Ëb¨¦l?GôÉÛÑo?t¬è•Í¡?r]ªÌê'?Ê+÷Á?©™Ûëø?'D²¼ÁÕ?…5ºÛÈO?¡¿b0'Sv?¦Ù¤"ƒÓ?íe^Ì  
?¤d™ž"²?'[ÎÀÿ"?Šóíýõ?°~CëN¿²?¡W¶gM~«?ëX9~Uy>?¬ß‰ý¥Z?evl.#é?€$¶ûª?ÁˆÂŸç8Ë?¬£a6²)Œ3FGL J0613.8-0201@jMõ¡lèÀ"—ô|ôÀ8
¤ž°ZÀ;#wÀOç@ÿ…$'@<ó%|?þ5لÁ¿¶CÛ2Qr¿ÜÜ#€Òg/¿ä°·•­ü¨¿ïJÑz kPSRPSR?sŠ$qÿ¼?x|tôñ%e?iyö?"b€ß?ƒ¹l¡¤z?v§÷ãç€?RÖÛ×£°?d¾ksI÷ô?ìˆ 8ë'?Á[É¢W÷å?»s£ÆÚ?ÁP~2D—x?šº° ½…?'K
ú
á?ìoe1_ê?£>qkò±?µÖ+†EŸn?ŸLZD«2þ?RZ£9ß?sS"
Š?îs©ÜšñÄ?šÍhé¨Ã'?¤ã÷êü|›?˜e®â:ûÇ3FGL J0614.1-3329@nà`þG™À5Ô´ßp=€À6ì^'À:œÆä@ý#¬¦@u˜>¥­#?þÞt§Ç¯­¿À'ª~nE¿Ö…¦|X¿áXez`Í¿êz¨Ea'žPSRPSR?…¾—ê˜\–?"5ãX{óè?íÚ¡Z´?¹»ýdë8'?°ÙW÷×TL?¶xÙ?UhvQ"†ð?r9Ng•?îß>xòÊ?¥ƒÛq4·j?¡`ÔÍ7¿'?¤é%êé|?»˜›™Þ?ªŒª$G6J?æ.œ"…ö?ºXoÜú÷&?ÉyAð…d;?³KCµ´å?PÕô‹g÷?QÓdçý)?îþýàa/á?–Ÿ…ÛT«?Ÿä«)MH?–Ô¯Ì<p3FGL J0615.4-3116@mÊòŸYÌûÀ4ՙÀ0XÀ9Òâ7˜ÂÀ;ÇyÒ9À'«0ð¸º@:ÀÌäIÁ@¥@¿ ¿é_äy'¼V¿å…Â+¼¥¿á"",zåØ¿á¸]Üv…eAGNbll?ïì.!ê͏?idÑ»n?@ø/θéü?I"§ù¤Li?_'¤Ciˆ?gEZ"J?ïÇ(—ú?x2¢öž"?ROwz½È?UêLËr+N?wê)Ö$AY?u¢K´•Ãþ?ïZw…<ü?Š«­hC¾?€‹5¬onÁ?o56•ä!—?–¯9 ©.?…†
EBœ+?ïÕ"V&¡?qMiü³œ¹>ëøE%¸ù¦?7«Í:%?uo9²YÒý?qFD£M3FGL J0617.2+5701@c­UàqÅ?@2ì_9K{À90½7-"À;"*m'ÓÒ¿úSndzÞ>@OYãÌÆ@T?b¿ÜsOa«ÛT¿ä1T>y@¿Û©NßG^õ¿ÙÛË}lg\AGNbll?ïôL®ÕH?S_û5žÀN?3Ñ/àµBô?.ìÀT0ñµ?RrV]B…ì?Q˜™ý´¯?ï›~¾3s?•wrÃÆó:?bEe 8G?gIYcä(.?"Ž÷-•H?"åfl±Û?îáH©èç?'áe<få?"jJŽgº?{ãPzÒ=?™ÃAÅ{¯n?ŒÇ¾æ/ú?ïžàÍ["ç?ƒ¡ýÀ@U?‹°0ñ·?Tù5º?ˆ4@ùT‹?ƒ˜=hvz3FGL J0617.2+2234e@g¡ŠŸb0@E?ªºÔÀ5iL"=À9¯Õh|Á@M1;ŒH"@d³kýª?ûwohÁh¿ÏDô¦°ƒk¿á4U݂&¶¿áW35å?¿ä鯁7xOTHERSNR? ~řüª?¹WÍÜsR?Û4ª&füÆ?ÏÜM¿ÊQ?á]¾",¶ü?ÐÊáϨ¸?M`È ›?oÞ–W«?ëѬ†(?Á¸)ýg"W?À›íäâ—Õ?Á£Ž§;?¹u#›º?¨¤&ÄâP?Õ¨ô5p:d?³e)Áß´­?áüã€å¯W?µôýÒCfQ?^Þ`㍚Õ?bðå
ìèÆ?æωJçßi?Âz;¶í}?ÒB	L³"?ÂcAgdLh3FGL J0617.6-1717@l¨ŸÆÚEÀ.1Ïþ°t§À92éf`‡)À;PñîÅE¿ç`Úö±!Ì@­À'U'z?þú¤¾æ°#¿ä6À'«ZP¿àb
¥^ó¿Úmœ;èí¿Ï¥{ÔP"…AGNbll?ïøXÀô?F"?ÓEPÉ?>ˆÓs»,?ö-Ú}µ8?K.'‰¸t?DhÞ2?ïÅ…
?}"L]Ö2Á?S'ámÉgÖ?Xõ9<Ó?x¶âŸ£?z€	‹ø<?ïL¿¦`8¶?Ø™Ð×?|QmU¹?r$‹–7iù?Ž§_½JS?zeªðPõ?ïu=9/è?syL*?㏇J0?bæ,¥Ê?'Hgv^?i@~ÿ'Â3FGL J0618.0+7819@`õÖàL'@8Üz¿¹¾ÓÀ:ZÍcˁsÀ<ÿ¼ä?娖×@Âùó÷^@ùÏãJ=¿çÖý3¿éMb˜óμ¿Ú¨O‹1U¿â/p¹"#AGNfsrq?ïê	<«DF?p€:Æç?Pî"õ
Ð?dè©>†?Zþñ´mjÅ?a	¢µ@)?ï|>íõ5?Ž&jJώà?¦gÑâªK?€—˜W?²Ñ]±?…ô¶Ò"—?ï!r½'já?Š©²Z®c?ƒ° U³k?|ˆºÊ
¸?'ù˜L‡ÊH?'bº,r?ï
Šö£+?"P¼%Ó?{€,jqky?~‡k¶Å´u?˜Þ£†?ž?'QõãÐ3FGL J0618.2-2429@lü1 žÛùÀ1Ï~¶ß%À:›¹.ŠWÀ;ÆĹØÔB?é4Ê]9tž@Ì9¶3k@U'1>¿ß¹Xôk—¿çöçMµ6¿ägÄäÝ¿ïÿ´ó‰œnAGNbcu?íqÇûߐ-?¶21Hžƒ?•l"s+áU?Ÿ™«õîá?®-6ˆq€?²¢f*ò8b?˳á@Çë?ÂÉùi"¬?â›oÁo8?Åð@¾¼Pð?Êvß¹{7?¾{Õ®"'?ê10öîú÷?¨œµJ¢äg?µúô*¬"	?ŸE †·?¸{"ەA?Ÿר8¶?ؼÞö®2?¸8¡hÜaF?Ú?BðdLÝ?¼õ‰vï?'1Ûcå?±¿4³ÄÚs3FGL J0618.9-1138@ky /µÐÀ(Ø´¡\ÜzÀ9•o"'ßÀ;LžáØÀ¤ê…š^@	Ýr"rl@ÁƒÿÔa¿ç8¨¢˜h9¿åjŽ‡[˜¿çMû¹§ß‹¿ç2uâ@ AGNbcu?îô©Œ¸–? ¾Z†´¼©?‰æoøvY;?'‹·è×gú?"w–ƒmÀ¨?˜¢§†d	?îߔnn,?±§ÛiÕL??ƒ¥HBlØ? Œ™Ûo‰ƒ?š:Î1ãû?§3ˆ£|"?ë¿ÂtÛ
?¥B‹ªñ	?¤Î$ågzÆ?BÁúb:?·šÙìÅj1?¡Ç÷Ú¸&x?ë؎'‡¿L?ºBü&Ò?Q†d‡È-?fpï"Þ­,?Àz¹•ó>?ºÛ̳úš3FGL J0620.4+2644@g6§?tŠ@‡'ŸÐ€À:F…íë*†À;ƒÜÌõ¹?Òi)ðûfy@µfEjC?úfz€NÄß¿ïÿüØ`?ïÿ›ß*ž¿×b÷ÌT×É¿àîúz¿	AGNbcu?ïìÊvuhñ?eCӓ)~?B±ã"n,É?BÑᚒ´?]!Kwò?c9lï¥?éCÃÆ·V?ȳºÜC:?­Ce/ËSœ?°áÈ<ò©Š?âã¤òM¿?Å.ôá¶?î?áX7=?•´¤ýGý?ŒP"YûÒ?~0S‰uG;?¤íä—u¯ò?"]®‹µ¯U?êžcYOb?·+b¨N?¼.>Y0?³CÀÁ£2?®	nR¾W"?«5ºFV‹3FGL J0621.0+2514@gcRàãG@;îN.ŒÀ9:ÛWªÀ;:‹#µî?ôø / V¢@6|CG}m@],¿ü"Ë?﵂·ï‰Õ¿ãèðjwµ¿Ý4À£ý¿îÜy'Š~PSRPSR?«àiˆÏRT?¥‰JP'?â¸Æ{¦Ý§?ËWwWb‹?×eטZi?ËážYù$?¢ÈþJEØ?¬Ú¶b|P?á*6oö?­?Íͯ_L?ÛRÀJ7í?Í·7莅?ÈþQ19'?°N¨Á<…?ä/9ÜÃ?µ*ÆFWÎ?ÆåfSb?¬F±®?Äïî¦6?²£Ž> ?áÒ¹ât8ï?Ãü€µ·Õe?ÑâÃÄ»?À=£Ÿr3FGL J0622.2+3747@eüãŠ	@%éW€•ÓÀ8¦'¿aª?À;…h9¥=<@4ڇöY
@èBæ.¢@Õ.=Ú¿Ó¤ÒrS.¦¿åcR§0ŸÊ¿îg
ɐ4õ¿ïþàf˜Ì{PSRPSR?Ãñ%£¬q?ȓ›p©ß?鴙Í(¸½?ɅÊnv¶?¤ñÏ&åÂX?©®Uexӈ?a¤" e?s.Å+t%ø?î!%¾	Ô?°à¨"ý8?­ƒ¥cî°Á?°¾%+DÙ%?ɤ¿SÒ"?®'‹ómœ0?äUñ{?´²Š"F@G?Æ:ÐjÖ?®qŽËrÀ3?}|`6²4'?u@©'Ò!?ï,AŒ4®?˜(ïÎM)?"¶kѝ?•`½<ñè3FGL J0622.4-2606@m:†
¢À11 ‹ü"À9u™	PâÀ;Q­nb´*¿Ý3šfž±@ T^Q?ÿÁÀTCy¿ã-¥+ëb±¿àøÐ_Ã"ï¿äª!|&—¿"/YðóXäAGNbll?ïôÌg=V¨?Su–Œ	?\IBݏ?V< žÞ?Tálñ$Õ~?Rz5¥b†Í?ïÈY$Ã,?{øoÌ?R§¸Æ
þx?ZÌ¥zæ	8?w)læ}‹?w ))Q|ú?îùUëÁÎô?gÞل'?ƒÛ:æé‰Æ?zÓø#c±?–ç¥Q\œ?‡ãGW͓S?ï¼øß³ö{?wËl&А×>û-""T)È?	lÈ`??€´1H¸7?wÅY—Idû3FGL J0622.9+3326@f~¿p@"P(ßó>À7_ÿ»6¢SÀ:¾t_Mm?ñmóþ¿ä@ $¥Z—ü@¿"|üÕÔ¿ßô,.©ƒ¿äʳ¿âÑ£˜˜_¿äŘQ´ÂYAGNBCU?В±?‡D´ØC+?Q0,º9'?Nl€É?†µ÷4"!ä?†­("Óá?ï!RÅGG?šñÜÚSÊÎ?^$Ù%$Tj?g	\‡Ö?‹ó*	£±?™¡>]'?í_u+V?¢§3´&Ík?•i˜£ËÚg?Œˆdꅴ?¯Sàüøu?ŸF'8z›?ïþ!•ÉLR?<ð|öµ  >šÖc'å¾@>¹Gü[Ô¨y?-Ù89qtÑ?<ì¸xM-3FGL J0623.3+3043@f͚€If{@ ý_çœ1À:,üۈQsÀ;«Ú
þ?ç#½É_ì@[ۓ9-H?þJ/ßÏ ¿ïÿö¡BÁ'?ïþ¨©Ú¼?Á¡í—÷'¿æ÷ãÃ÷€AGNbcu?ï›™@BS?'X×öë§Ì?d²#§?e¿Bof0?"êE¤¢?-ÚNõ+¨?ç2WàŠLÕ?ϟ{µ]4?¼¶=:X?Ä5þnB#e?Å.Å_V¯}?Ç@…"±
?í秶•`ä?¡{íå},u?"±Ù9»+?ˆÃ®³Žù?§¬˜
&?œEçƒ9ã?í]µ.^ "?´DvM†?ªóO4e»?±Ú;0Òâ6? !¹Êá'?¥G8Òë™3FGL J0625.2+4440@e8OïI@,ÈFŸ ÂÀ9`+½,aÀ;'½ÝEÀÔ?–HDƒw@ºûø´\>@^È b¿älAÒæÊØ¿ãŠaçÚ"¿ÕÑéÝ­è¿Ý°6ÃOd[AGNbll?ïÎQ…^K?}jã¿Ôþ?G_'Ó§Õn?N¿œ8¹]?uëXƒÛߊ?|¹֚ò?ï2lNdY?¡>ûTn?rØZþ>|D?r»ÚùâF?—Û¶£Õá? Lè´0¬<?îú;­Ïß?Ž€|s²ë?ƒ¥6B¡?x´`!k\?–åï<ù3F?‡WaºÈ°‹?îÛB®±*3?'þDÞ¥»?UçFŸ˜O\?YBJ§Y¦ä?¡œšßðšY?'©fú•3FGL J0626.0-5436@pu¨€QÉ÷À9ac€X€À9§Ú¥ÓdÀ;Áw=N?(?ÑÇÓÔ(
á@ã&?YÝ@]Ϡ׿ꬽo%–¿èñ2Á¸
¿åqh_åÿ¿ïþýR•gõAGNfsrq?ïø¨D™Ø?J4¯ÀŒÁV?3(
×Sh?8ª´Nl¼?CÊ®óü?DæGOÙ?îL™Ög?®Íêõu?'
Iþ?˜={Gþ^k?¥¦ÝuE?§/ðe¬µ?îûB
Ã?Œ;pèQlÑ?^˽†š?'fWÝ:?8ò¢A€?€öBg EŠ?íK˜ÎmÞà?¥î¤å-•?—À/•òxË?ŽÚՄ›f?¯f[N(Õ¯?¢9	áv3›3FGL J0626.6-4259@obY@x–À6hŸä6vÀ:!¾ê‹úuÀ;¥ðÍ]…?ôÁwAU
@¤f&O ?ûÖÁM½£¿æï"VZïT¿ÕËèÒ£ĿƝ_d‹è¿Óś¿}r¶AGNbcu?ïO
$;LÀ?™å4{[ˆh?‹s''¯?"g*Þ"?$£}ª¨)?…Ü#"w"«?ïNkîM?œžZ WF?r¬ÿas—?|‹p¦P"?'‡Oý¹¨?—ˈ¹ax?槲Vì?´Á"1¦"?Å\ÎßY!?®cø×ȂE?Àh†p8£?ªÁ{¦‰?î@_X¨«n?¤¾þK5#¤?'¨õÌQ¸?J»¸ÒK?¨ÕV»¾Ü?¡ÎYހ"{3FGL J0627.0-3529@nnƒ¡	ÐcÀ3øÄ!HÀ8ÎFªß<;À;*½•!dÕ¿ÐÓT;ý˜X@=B´Z?ýåS ¹^¿ç'chP¿ÓS0¹±<#¿ÞE]i‰þ¾¿Ø @…~bAGNrdg?ïÔ#ý9ÉE?pæø?è?SäônÐàÔ?XÖ<Ìژ¶?pôÄGg%M?lýºÆXÈ-?ïž+Ŕ‰è? ©•s?b&׸< ?du¦`Ư?ƒëX¬Î]Û?‹a~"Ñ{3?î2½§/;?šl{™ÈÊ?"ŸqÅÎÜþ?ˆÍ'…#q?¢"mB¥Ð?'ëä@Ê"?íúíqïGS?—¢çŒÅ%?Uê^Ât?X‰í€eÞÈ?¯¨iŽz?—oùĒK3FGL J0627.9-1517@lãø¶À(hß½jYÀ9óEî ÚkÀ;p©Ã³H—?ãÎöZS#@µú´¼Šµ@É£àDxÖ¿ãhD"œ™¿ï;Ât•dg¿Ù‡Èö?ÙÜç&•@AGNbcu?ïٚ15Ç~?zŒk–üz?9ó¥k+tÛ??Ö Ø!w?q"­i‰'?yЗb>?ï+²Ì».²?²ûY"Ȃ˜?rBz·3·?ÙþFì‹?•ùºÍ;î?°B'0JG?íÙ:D9&à?PNK(ƒ'?‰²£»§¹?zec_¦áT?«ÿ²Íƒ£´?š¬A—Búd?ïW>tËÅ?"Yt…·#Ô?5,ٞø>?Uò:¶!P?"Ã~Š¥?"=x'6½3FGL J0629.0-6248@q{`(^ÄÀ:oc€X€À9ʉŒ\`À;ÏXK±?Íã¶ÑÁ\@ć®à~@Õ$@Q(ç¿ä}©kD,¿ãA'á2y¿âЅÛe…°¿ÔsºH!AGNbll?îë3Ö?¢AXŸ)?fb-½ªÉ?g-\po`?ŸÍDù8hþ?¡ºMeÏ̇?ï^Ú£ aÏ?"'¿ Ï¡?nÅ
¾3¤?t¯œ>¾$?a'ê;ÿ¶?@˜/µÌ?îO'?øž?–	ãô÷ó?9oñÊH?^îv8CŒ?¢ê4?''	?(Kg_¦?îªÑ$'ë?–-$À"è4?fA¡8åŠH?kµŒ;D/?£ú˜Ú)x¸?•"Ó<G]3FGL J0629.4-1959@l"†_•'ÍÀ+Mûþé‹À7ý0T[¡çÀ;A0Kø&?íªJ
aµ@NkåuF@u'A8¿à
øe¤A
¿äuŠFHx¿àˆM-Ê¿ä"'J¿ä)AGNbll?ïßù"ýÃú?s)TgkV?=;6"ýR?=t6$Ä33?lf›keÕ?rŸ\72ì?ï¹&\äÿ?'²:=Wª}?V‡µôû?\u¾G\W?}ËPBT?€ü¹ÎL¼¬?îcºÀmY?–"Ø"M?Ž
Gÿ¿e'?'ÒèE©O?¢AÁþ)Q?'OÔcoe?ïžÁ±W/¤?"ô•?'–@?*u…8n?5ùŒ Ÿ€%?‡ç…Ô5D?"è9šèÆ®3FGL J0630.3+6906@b6`RP/@7b°ÿèÀ:ŒçìãÉÀ;úÌh"ÿ	¿ôßa.Ä
¶@
ÈÖ\˜‡@$ÇÛØX¿ã°»Ë·gпá´å]ÍÞ¿åR=‹7u¿êf:3Øt¡AGNbcu?îsÎ͕M]?¥Ä/ח?¤Râ½£D¹?¤};êÑ«ä?ÀÁ¤•´?2-»$?ïÏVp?¡,ß­_?¥?ŽQN»¯ª£?"ù¾Œf?Œúð®´OÓ?" !â n?ìÓM©E¬Š? £Î®|¸8?©LÞÊóä?•tHsRf*?©~F ²1?"]|Ü®#?î¡ Šàß?›'¯›ãî?¹Q%ÍÑ?…µ+ƒ7˜Ë?¡öÍ-8lš?—UQ÷«J3FGL J0630.9-2406@mí_‹ÎÀ-úðþÛ<ÒÀ7ßEó)WèÀ:°3cÛW?èÚ^t™I@—v2â*'?üó'_?€ž¿ËQú"Úgë¿Þ~OñQ^¿×¾!K²¹"¿ÓNÙ|ˆ'´AGNbll?ï?Yâc?‰cÀˆ%š?ZÛCˆKÕ?aœAOÐ?…TÁH>v?‡ÏøÙµŠŸ?ï%™Tvò·?¦!{´¹?u	L¿ÅÓ?M¥(Ò?–
'A04v?¤«êD™?èÒÕôžÚ?µp!H¼ˆ?¤<÷xeƒ9?™?.¿Cq¶?Ç¥mÒ#Ê?²Ã>dÞm?å–î^Âc
?µäƒxÂ?'¨dA(?ˆb(}	.?ÔF
ÿY-ã?µÓ¼®î¶.3FGL J0631.2+2019@hêßqêÿ@x€0¥À9fۙjZÀ;˜K»À5¿ä«—Y3´@st:9Œ¿@®èŸf7B¿åšqҚ¿éº€6œY¿á¿3]¿<°¿á¯hþ·_AGNbcu?íZ¦žMҌ?·§¹Žù ?W2Oæß?[®913?´ÎŽDQÓA?·ƒ¢Îþ6¼?î1m¥?¯cˆˆ'è­?p6ÓSˆU§?u¸av	<"?ªâKEu$ó?®PÐ!??ëˀ"Ö?«&ùÁa?œ:qº™·j?'ÀZ™¦Ç`?º•cLót?§b-šÌó?íƄä¸çö??²T`_ ?4š¦oç?3<¹T/Ž?±·>3É´B?3ŠM>ž3FGL J0631.5+1036@i's`Iì³?Ýær¿~õBÀ7ö†
˚žÀ:ÙҢϣA@– ´Ö`õ@
ý6E'@?õ8{Çw¿ÕF
ë_¿Ý.×výk¿âžržzv`¿ìO^\#8âPSRPSR?OÿÎk?L§Y4´ªÚ?î&ý'gr?°tb²ŠÍá?­Ãã–OH?°Y7)ÇÑ?:›JXjLž?Vcã*v›?éÉÜcțV?¿Î/"¿Ý?ÈË@˱]ƒ?¿
<~TV?–Åwæ*ýt?‹-\c…~ñ?뿈"óx?¨k@	®"b?¼R]fـ?¥tÒe_êý?‹ùD$t?7‹%À1?ìƒèO?©"&Êöê?»œ½Ôóç?¦åk'¨ñM3FGL J0631.6+0644@i•¥¿­)™¿ôàÖ¿"ÕåÀ8"^ëGâÀ:–½öp4F?ù‡ÉûŒ'ì@ø'÷ŽÂ?÷­TF©1½¿—Õž'ŒŒÁ¿âà"~¿á7ɀ2W¿ìŒ˜_ö"OTHERspp?K'ðmÀ¯?N[زhF?Þ²×¤]?и¡ýX?àò¯!?к‰Yüdñ?aƒDªñù?†dû@ӗ?àï–:9ä?̉¥|'ù?ÝýÍkV6S?̦³´Ho?§P—ôt?"¯¦Ç†%A?ãZ}mO¢?´Új†(¬?Öa

½V?´G›o¬fz?­¶‡U¦ß·? éñŽE)Ô?ÙnÕò˜ð?À¢"f?ám,'¢ÅŒ?À¤[8a˜Í3FGL J0633.7+0632@i£¿YFÿí»8 
•
À6ιƒCì¿À:Z֒Hl€@Ï)à#@Í@Vð9Žl@Ãë&Õù¿ÒSŽ:žj¿á0<<‹'¿æ9vTH¿í~Žè ÷PSRPSR?/'¡Ký]?1×`‰ã[?ïÔ~NØe?wJõ[]:×?tÄɗâ;?vô'jõ?ÓÂòv;?5.0ç‹R?ìX+î} '?¸cã^Å£X?½:Ƹ½Û?¸ciÍ7
Þ?}kàµÐ-?€µ=w€?ퟞxɹ?¡ÑË+FK?¶E.U1? xT—©a?Qw"ïé?Olc[§é?îsÆ~{«à?™‰eÒû;‹?¨7ۛ¥É'?™«Áá·3FGL J0633.9+1746@hdA¿½ð'@'H$\À3L­áO:ÑÀ9=XJ@Äòýãñ@¶¥¹7™Ÿ?ôP'Ldë¿ÀŠ(æ¿ÚeR˜[߂¿ååðy+¿îA÷~§$òPSRPSR?E¨S'ö?=pN>¿?ï=oJ"­?©O$"]‰a?˜DsÙTBA?©KîžZ?[ÔI:¸q•?"•>i­5?í·BK&ñ¯?Á¯'…)®?±ÖœÝÁ?À«*Ÿòàä?kdCšÕA?t&þô@](?ëH҃ÀšC?¬ìtPÉJ#?Âo$ä›+ ?¬Ò­A93ö>™Ê
ëw>­¿ÊO«û?ïå°çXdÎ?pûcð|cï?jNL)J‰%?pû ]3FGL J0634.7-2334@mû 1ίÀ+ýüߺ[À9£€)†À;ëˆy¶¥?欠tª û@?s­KÓ@JE Eš¿¿çm!W­TÑ¿åò¢ô@ã¿ëäTc ÿïÿL]?ýAGNfsrq?ï«l¼.ú?‡ü,¸ÛB?ð㹒.?"ø½4o>?eq|]à©?i……Ú̶?é%×Òn!(?ÄÓ"¶Gy°?·õ\[ÞýÈ?³¤²ö3 ?¾Ûå¯ù?¼
`AÀ4Ø?ík_€9À»?­d	Ý?¦Ä3žs´?•îֈ±?¢…Ô]ðٙ?Wé8£Ð?ä|txÎ÷'?´*²?ÉR]£=S?´=99 ð?Ä»Ðy†Î½?¯4sù§ÕO3FGL J0635.7-7517@qæG rѯÀ;)_JsÀ86
ÄÀ;•« éð?æÅ]‰ÀU@eºsY@®àI+m¿æ¶{v1ÏJ¿è]¦öh@u¿ë,͑Ôå[¿ïÿ.¶÷£eAGNfsrq?ïøŒ<ú?F«dÂ˜?AïQv¢´G?A€n¨¤ou?7¿|âê3Æ?8"—3.|?ï±x›.ç?€»ÔJÚì®?[¾:y¼?bÒ­¤•?€?Am0ŽÊ?}P>ñS^?îܑ֖Œ[?Œƒ/uÙ?"ÉS¶Ä?"N7A<h,?'cз
\k?@…&;?ﭏqÆÀ?‡]ýBñ'œ?X)wÆ·q$?d=hr@õ?–ô•£b?†¥Ñ,©l3FGL J0638.6+7324@a¨ Àiçû@9¬OkxÀ9—}K…9À;ÝM×#gä¿Ñ{Ë6Žv?@.²§²Œ@笳¿æS<ã¹á¿éj;ÿE׿ä=š?\¿ïÿ©ü=RÇAGNfsrq?ïþyè{?.Æ tÈ?gY-?"†A|¦¦Š? ‡§ó#Q£?&gÓšŽè?ï³,¥¶–˜?'šFXΦ?niÝ}íÿj?p9}ïû?w4¾e½´ù?}W°÷2'?ï?Ön3£e?‰r¶¸y;ý?†A#†Z&?jö¦ÜV?‰É@ì½I?ƒ.³Š—?G?ï¦>è½$c?ƒ=nAx2]?Zë)nSi?_è±.¹¨?ƒ-èk‰¸?ã¼$æšù3FGL J0640.0-1252@kæHÿ¸²dÀ ŸóI"À9æ´5&RÀ;UHf¡?à9¶{#@
ÔÍLN?ø3@¿bÖå?ïò>Çøþ¿àV³üyì3?Ëò«{ã¿ÌŸÀÿRõµAGNbcu?íÇ|žVÐ?¶
܃OС?dŽÕY‡]?†áº»ôI?±¤g'}J?µ·@Þùãf?î疆ûV?¸H.7NA?ww§"ZgZ?ƒ$òùÞ$?¬'³DýÀ?·ª¤¶HÙ?íQo¨_RG?Ÿ_Ëõs5ï?™älô‰?‰Àú۟}?®"DáM?™Ë
ç«k5?íD×Ìôü?ª´q?M½ëPÖ-~?a»¤‹?µË:ö«Ã?ªÀÕie*3FGL J0640.9+0752@i—]÷vÅ?ô}^?{kÀ9Ï!j´À:Í"4H?¸Vº£‰ÅW@
]lŽôz@rZ¿i6û¿äu§L
¿êÂ]B¡¿ê)^ž	¿ÑÒã|¼"OTHERspp?Ã"2Ì?Ç+5°í?´Z­¦µÆ?µŠ#­?è¬&cúŒ?ÉP»aÜ?ÐCù3¿ó?Ðÿës‹Ü?®"®Ë1©±?´Äß$Õ)?åôÈy…k?ÐÆȑ1—?à\·F{ªN?¶(oz·?Â<=?¢o?¬$ö^•‰¤?Ö(‹ThÚ,?´ã¹ "?å+Æïâ™?Áh£¯Ù'õ?†óss"·?ŒFêHÑa?ÔðØJ‡&Q?ÁFjaÖ-ã3FGL J0641.8-0319@jÙ¦ %9uÀ
gßbP­À9‡86¨2ºÀ;¯#nš?çÞKpåW@¬¡ÚZÔã@¢Êi²K¿æZ×ä⣿ã=*É(å¿ãÀãîZÙ¿ïÿôG÷ ÅAGNbcu?ïWû\±^?±JFÀh?wÅWc°
?"/n¬¬ôÍ?Ž'7Т?°ºÿó|à?äéH\.?Ðù˜Îã!
?§Â;¨±î?®›)4öu5?Ó5û'‡?ÎÍ`*ó^?éæè'žº??­×fý«¦?´žÏK-h»?¡f'‹?¼)ïwÜÅK?§¯i+ý!?ì¿a*Vè?ªÙWâƊ?†ý±Qÿþ?…<ƒ
ò®j?·%@ƒåB?¨-ŽD `3FGL J0643.2+0859@i®ÀrKw@:ßkàÏÀ8dbzÀ:ÎÜq…~?ùûdg@Ú3më–@ÜN®¹¼O¿Þÿi;Ö¿ä»`ã¼õ·¿è|s±±¿ïÿ…"
ì'AGNfsrq?î`8r·?°	Ï.W?"Êô6¡?°?š'($›ø2?Ÿ.ûßÎ?ªµJuL 0?êW¨Z?Ǩ
ÞÓMª?•v³©¢G?dã˜oòæ?Ãò‰ƒyc¥?ÆKÁorچ?â¼K¬?p?¶÷Ò#Çp'?É!Ãèμ?­s´>>µ?Îc
f3‡?²òdLtK?æžN"?½BUì?±LT(ª?®‡œj!·?ÏSƒ¸³œ ?¹Þ¯K(3FGL J0643.4-5358@pu3?ÈlìÀ6ÆfÙ×À:
Oa´À;Ç1Xg "¿òó—Œy§@Ùê†7"@Œy¦Žu¿êN=ÄAôþ¿×%ƒˆÇJ"¿ç½z_þ©z¿èñ04;AGNbcu?ïÝW¸Ë=?|ࡎ¶#?fAø_6(:?qèåLÀ?YC_Ïý2s?pŠj@ʊ?ï³à‡»‹Ç?"žíË,?WÊÖºˆ£¹?\Š1ò?€ƒ9Ëù ?ƒ"OŒõ»è?î¼£+~¨?'6ŽÙ#]¸?"u܏-v?‰ü&¸Obø?"	"ý‡?ƒ`XaLuj?ï±ÇlŠ?z~uïõ?A¥H³è'ú?QZèͺ?'žù™ºTÈ?x‹N45°3FGL J0644.3-6713@qX—ÿ›V2À9‰4ŸCý†À7ØýCŠÀ;åÉä?ìD™ùw@Ou¬ªm|@ÂÿýfH¿àý'²Ìq¿áæ
n £¿à½ëtœxá¿åS
æ&ÔÅAGNbcu?ïôO&Àe?Q|}Òà%?0š™ü(/¯?1c'È»¤?S;+í÷?P}ŒÌëÛº?ïÆÿÝ$_¤?{%"V¹VÇ?O+"nz:ö?S~Påû?xšžàæ¾?x®Lµéma?î¼wû†Ô>?á_d¥W3?‡Ô4ü0¶^?<¿kÖq:?œ†æ
ò?ŠùùÀŽù%?ï߅fo·?sPïpn?'*+ƒ¥¨?ÜZU°»?p*œñj?s<…cæúÿ3FGL J0644.6-2853@mÏ:ÿ°NèÀ,.z WŽ\À:_Ï2ÚÌÀ;Ä}‹F¿×{ٌ›%Ø@d‹šÓU}@㦿qð]¿ït¾§VVà?å	k©qRþ¿Üù»ŠA¸¿ëP"T'±AGNbcu?ï;
>e?¡úg;nld?•"(7ÆZ?™	 !ˆ/?€èíÚt ?•Áƒ]žG?î ÕP
È?©4ÚuQ?‰þÎh­?'àh5µ"4?žåîÊ=?¤N•mÅ?묢,B ?¨B³û6ð?¶DÔÃv½¤?£§¿Â;ä?¨µÌVNbª?•*ŸiÙë#?îø¨æ«S+?ŸøÉ®ªº3?'×8¿$X?šçY
~?Ž'ã¬ìF?‹gTg"¬3FGL J0645.9-3914@o@ßXÀ‹À1À¶àÒ=OÀ:ª>,‹À;Á¦V]ÛÀõ‹¾åƒ}@Ê'D½t@'ù gÔ{¿êI»üke¿é
šO±™¿å«¤¶£¸¿ïÿ1¾¾íAGNfsrq?ï틻	¢*?e÷íÛVœ¢?MK]ûõæ9?WäpD­h?VBÚîÀ¹ž?]UuÊ 
?'†}Î?""óù+¾?d< g	?sE´¿¼a?…–Œv<²¥?'vìe'm?îþ?ÁK?•^&\±"?žéëü /?Š`O\mM?  §
ð??‹Ê3úô(Ä?ïw?®ÎGù?'×^Ž‰ôR?4oٜ¬Õ?SÖFËf°?Ç¨fЍý?'éuÑ3FGL J0646.4-5452@p†Z\FRÀ6˜À§¨À:±Œ7±G5À<w&0ì1?öaÖâOj÷@!VØÿ¶¿È]¢Pþ?ï¯ù͋äz¿ÚՕŽ7ï¿èÛ~re'ï¿ïþÞdFHAGNbcu?Çn[\¼F?ÐÓ°¡è?åæÁþà,?Ô§«a%?Àöœ«Ã?Î_ÿ
®‰?»È¯Ó;0?ÆÃZՌ!?çZrÙ?Îljƒ6?ı߶Í!?Ã)Ê©‡"ï?ÅÙŨ5[Ò?°#ã½;ߗ?å}úÖ­'?¶Äu1~Z?Ä.RToíê?°h¦–ñ?ÚðÁdˌn?ό«Ðšâe?Þ¡­
¸ö‰?Ïw澅ºQ?¹¶F5íô(?Á›ÃÔÛÐÐ3FGL J0647.0-5134@pOø!ïÀ5"Ð_ÿDÀ:C*È*§À;ڈ§ÙÎ=?Å$ÿÇSš@
âÖ¤fý@ƒâ?Ð¥t¿çÈÓ*^¿æb5a¶©J¿Ø–8¥³%¿ÑyFðKÏYAGNbcu?ïÙ«¡f=??zšÒH?Bå
$Œ?RL›±?pÍ}L?¼^?xœ \üž;?ïL¥ªDlz?žÀÜmԗY?s2'ë¦Qò?'}ppޒz?'žÀ¼ˆÜN?—x×1
D{?î©Sʯf?‹#cÂÀë?ˆ5-/Œ?uo¢äƒ@Ù?žÕl!ü§É?…EÞ°ýœ'?îΖ$X4?"Tîn#'?TÚ¬"ÏEÅ?clŒ÷=?¢oÈ]Ô¡?"òB=n'"3FGL J0647.1-4415@o²Í ¯¢ðÀ3I`ÆuÀ:œç+ó¤À;ÙLhÏÍ?¼ýaÄYûc@]†ÎÇ8@Ás\f³¿ìôyI˃ª¿åÐhYíî?Æ ?ïìÒRzÌ$AGNbcu?ïhsŒ,@œ?—eùh×e"?"ׯŗx?2{:G]?E*A‹?…Bú¡?ª?íHT¯¦½?¹¸0B? ¹kð)[[?©úĈLä2?ªÁIì8Ù?®¡aSr]|?ëÀÇm…ö?¥©u}y¤?°6§\‡Æ?œ››Ï:??±Ã:ä
I?›ú3Ÿ}5¾?íhg"Ëšº?­uII;ðs?y՞¬Çµ}?‡3eÈt›%?³iîÖ®Ï?«îSúª¬3FGL J0647.6-6058@píοìºÀ7ñàè@À9KTÛúg:À;­ÈŽyªç¿'t8w÷@ŸŠùB̃@±¡ y1ſޟÜaÈÐq¿åd'ït¿ä3Æ£_c¿ç,=¾&–ÃAGNbcu?ïëöztP¼?dÇíJ<Õx?B©‡÷I?U@ÏQ;?^¾GÕ߃?Yèe!¬Í?C 8{?†e…_	‹?eп"þ²?gâò!œ^Ú?‡ã¨h)!C?ƒdh\8d1?îõñÀ4?ˆa¾éïÇ?…½~ì1?we!ä¹?–²ýèõ‡"?€²;¾B`?î÷ԟ††‰?"¾ëƒó³ÿ?a®Î§þô¹?^úOÎî?žÏ':/PF?"5ëÖÚÁì3FGL J0648.1+1606@hÅZÀ?ö@A.Àë­À:…Ç7bÀ;±'[¶¿ížðÆ|&@SöâŸòÏ?üdÞßHûG¿ë\Šfd§¹¿æ̶Êàl¿ØHZ¾"Ì¿ÝOŽéðÓAGNbcu?ïñò•yYl?\[i'Rd?&L¼!"È?)ëT-Âu?YQ=‰+6¯?Z''B[>"?í'Ü­	Me?º¹êã›?wÎnyõA?ˆ¡ŸÃÇûÀ?²l3°@¸?¹ˆÉnŽ÷?îmk뤟ø?"5¨³J,?…â¼îë?u+Ʀɋ?£ÅÂÆÄÓ?'1ÈdV"?+ÓÖ?"%maÁ£¹?*!@d}Uã?1%—Šý
?Ÿ§¹¼Š?"Õˆß3FGL J0648.1-3045@nÈ˒:À,BIÿ''ìÀ8áfãcèÀ;rÍ 1cO¿¼Ü+Ë­4@GÜ7£Û@te€¿æ#­5F¢–¿èZçï+á¿ãHþ®òf¿è»zóoAGNfsrq?ïùÎe͸?I¢n#üÓò?ÅE¤U?®¬#ýl?HÜÅT¡
?H"ÓkÎ;½?ï̯±*?{j`ÒøO?Ný|×<?S¦_}?vø¤}³?xð'd©Ÿß?ïd"¾œ
?""!Ä<?}Q7…‰+²?l0Ÿ¾Âô?–?¦Ê3µ?¿¶&Ñû?ïô¾Ž—o?ZS*OÍyq>Úé;íémŸ>é¢%¹?Vgù¢ã7ß?ZEc·ý?3FGL J0648.8+1516@hߚŸ¾vÉ@VÚ`SaÀ8ÄN¨¿¨À;ÚaàŨ¿èÞn3ÔÂ@­@͵€?ýKF(_?ÍF:™Pjô¿Ôl.[ ü¿¿×``¹Û¿Ù-Á¼î‹AGNbll?Ciš?¬Èl獧?ƒV–6wâ"?†à‰Ûà1?©î+m±?ª½L·2O?ì"éæ'ø?¼ØA%Õä?ƒèWô¯õ?‡7a1Ìcƒ?¸Û¥Ûi©ÿ?»g–-ʗ?ê˜QV28\?¬(ĤtXó?¦ÛþœÝßÍ?"ö{2¢0Ü?¿ÏuÿÿM:?§ÌYã³?é襤]?µ!žoY5?p>ðV՝?rçs,yŠ˜?ÇÁíCÓ ?µ£¶ô6g3FGL J0648.8-1740@lŒ`Ëò²À!9ÿÖ•À9aéÐé'ÿÀ;%HŽå?Éoà<+ø@¾ß"	v@(Mß[ð—¿è`.'ô¿ãÉç'/y¿éѼø»¿åº4!xSAGNfsrq?ïÙÊAƒ?wɋ±¥žÝ?W?š¨Òü?b@­'ìgŽ?kIhjëÒ?pÍE£u—?ïÝ)†r?¦/	T´?hÓrW?uôiô"ßX?šaXÔÛã"?¤!iÐ
Ð?îogPÏö?'I™-ûÞ?'VsK²¿?"Øä_à*?ŸÆŸÊ3B;?Š"Þ©¡L?ï?è~|†E?LÑ€'?A3ž>QÐ?E}´7©i?—yS>|®Õ?ŒùãS1øÔ3FGL J0649.6-3138@n06¿DNÀ,d:a$ÞÀ9¬þ›{ñéÀ;`œ
è ?ͯzVˆLë@¸±¤þ&·?û¨² yL¿ìýkÆLªþ?Þý*ÍŽØ¿Ãsýyy#é¿Û­fѬk¿AGNbcu?ïÏEíƒ5?€·vÖS?J"*^hú?F Sĺ¶?uع.˜™?€ZԜ"g1?ï]‡
H?šßìT/?q´õåZF?~äç栅?ÃÁ»tëq?•¶\-¹‰X?î¦(sú­?—r°^̵?Š–Ï"*S?{•  ãfß?ï‰¶ªH?‰³H†%??!žd7? ØHöiI ?qÿj)'Ù&?n\
¿Ü°µ?¥"à çad? '—±3FGL J0650.4-1636@lv²gÇÀÓþ_ìÏ¢À9.Wø™÷À;Æ폺ô?ðûc"xB\@håòŽ@uâÿi,>¿ÚéÒU'›¸¿æ[xt
¿é€îIõ˜¿ç¯£2ìÞ²AGNbcu?ãÓq¾z—7?Æŗ~»X^?Ìý=°¥ý?ÃhY…÷°?ôûUo¦?¾¾8²êP?âcè,o•ü?ϐEÀMo?»ÂÀB¿!?¹	`a\‰Q?ÔG–q?ÈAb(\»?çÆo!ðúÁ?°s5A…m?»‡ý¿iì'?¢,¤«Óåÿ?Ã"D˜‡»?§Ã©É=
?à-~Ÿþ?±Åaˆ#E¦?ÄÀg¬­•Ö?²ÈìÚ+ö¦?ÕDÎé¬÷Ü?°µ0ÏçûÕ3FGL J0650.5+2055@hA}`éNä@"c.Àë­À9¶'Ã]À;Th®?C¿°[5ÑÎ2`@«–ÌŠ²¡?ø@W¿ê»b‹TKK¿ØêpY·ßÞ?›FAi#¿Âôû#ÞAGNbcu?ï´~Â7À·?…c£4™»A?Sõ™‹ã"?`8ŒWœ^?€a­>ÞUò?"(UÞ£\Ù?î^ùNêÖ*?®ŽUu?q6ÚOôÝm?t®ƒ3M-?§éÇT¬?­Y¥Ç3æ5?îJ€ L†?˜ï‹é¯Øõ?F'S!48?­C—6•ÿ?¤Ca2ê€?•Zž8ãÅD?ïM›®ò‡Ù?äên¢¸s?7WIÓn˜?*œ¦æ_­7?–4RÊe1y?×5ö¶ý3FGL J0650.7+2503@gȱ ‹ü"@&ðál—À8F-ù7ŽãÀ:мž_ç¿ÞÂrYzH@ 9#¸?ûˆ~žìiË¿Ób"ý[>¿ÜυÜé-¿Ð¦=Y°S"¿Ôà©3¦²AGNbll?¦û9û?—ˆ:Úw5)?FKàmr_ç?RצÁ´	?ˆ¹:Z[Z?–™M…ë¶ø?îöÑ^YÚ§?£?€«4+f?mãµ#Øøh?qdIJ˜<?i]IŒ?¢CQÖkÂÿ?ìfXf'wH?§ëî~'?•Z×àZ?Šõú?›7"?·v¶ØÌ/<?¥r: üö?í257ÃÖç?¡©Ë6i_?7•RÞùº?D[¥bݼó?¶VÁ=ŽiÅ?¡›Á/ä(—3FGL J0651.3+4014@eýÓX"@1­ _À:«õ¼°À;ËÌ%ÝàÀlæ.D@ø{
bZ@õþ€y0¿ÕOÌÔâùh¿éùIЃ'¿Åš—ùäæ¿Ünf¶©†AGNbcu?ïù/öÓ\?\Ñ)~ÿP?¼‹-Þ?;Ü<l?IXqáí?[ÊCÒz'9?ïrá…b‹?¤ÛngÃï?aïWuӀG?siv]'à?ŽËÈÉè_?£–Îïá\?ï5;hh^P?‡ÁaÎE?}»µMÀ/?sãO6jjõ?'饟"*/?ƒ¬ÄõBöu?ïðN"ûg?^¥#0ÜÔf> ÏÔ+‹>²âÐ'gL?_`½ƒÏû?^£f… Õ$3FGL J0652.0-4808@pQ?´‰À3ÀÆ3¡îÀ:iñxôÀ;×PÁ¹sT?êº°‰íw@
üxŒØ@Z"`Ÿ§ü¿ëœ†ÀŠ/¿æf1ýþóæ¿ÝBÛB—f?œ^yæ~'EAGNbcu?ï׊¿¿žt?s5õt€I3?Z8î'4ì?`ÓyX'O?kXÉ8 pK?oL÷ô†çµ?ïh§Ð÷3?­Ä©Â©aP?zÀ/äŒ!C?'Y¾ñêÝ?•Âß¾=?¦ŽÍ¿#ãV?íáɶdž??š´(A°¦?™L¹"Hª?…¡ìbùž?¥=½wÈ?'–@@Ÿ¼"?îöͳFöñ?™•¥™óMÖ?fÞ­cr?"{×r%?žJsôT¾Ô?—­NÁ{¬S3FGL J0653.6+2817@gqXf€@)Ú'ÿ"ŠoÀ9£/…(ÉÀ;¶ÄnYyï¿þK_§…jŽ@èžd"@ÿâ'…¤¿è\Žab'¿ã55¬E¿ÐuÛӔ«ã¿éå¡9ËþœAGNbcu?ïudhÝù?˜P¹=ƒv?€\Ap‹?•\wãê,?'JºÚXp7?"¯…‰
Áu?îÙèxnr?«ð'X8³?qaøoʦ?zü·mž%? >³‰k"?©¾Ó<Oa?íøgL ú/?¡z¦Ö²?šÝ°
NÄÉ?':‡Rô˜W?£
³8Èú¬?'×$]Ï9Z?ï±Ò[¥–/?šžÞþhÀ?ÃÑeã?%tò+ýC?ƒcátƒ¨•?Ç¼*Ø33FGL J0654.4+4514@efŠá'6@3cS`Ð$pÀ8ºp©¶À;Vä'Ë÷»?ì²*3Uö@Vn=Í@L_ß¹Ž'¿á#±¿å0ŸZ"á¿ã[ù¥óÅ	¿æ¶ÿNAGNFSRQ?ïøEÿm?Gž£"X.Ô?4Â7"ÿ\Š?1KGµéÓ?EŠ·œD?C—s†×¸
?ïÏÌ4sý?€œ–¶¡µ?_R'\vq˜?dš¾KÙ·?pEA¤¨eá?|õ›´G?ïH-mÖÕ´?†°:Ç/ÑÚ?}b\Ò ´?t53I'š?Cv!ä?iíˆT?ïû¢õi;?Mfª{¢'>ØȜî¡">òG
FÆ?ABšl}ÒÝ?MBë$Ê3FGL J0654.4+5042@d¶êá‹@5w ÈÍdÀ8Þˆò'À;y\*£A¹?öŒ¬KMl@<³µ¥?ü¢õ°pÌ¿Õj=p£×
¿àËp¶÷M¿âmX•dοæþŽÆÚ
AGNfsrq?ïì¯òÈ/?_@Á×x2í?QšÓXÿ?M'ü<Û_§?V搜Hø?Y{wç¡?ïÀô¡3Òz?€ðx[Œü?il–UK?kyٓº"à?rÏ¥%K˜Ð?vòyo1yM?ì€óË"¸7?¦ˆìúFC?­ù ºõ? c¤nc?©÷¢"Ðú?œ½n¤#a?÷¯r?… Æw?_·ZKVââ?d$i,W@d?…ßVöiG?"¼;8Ž%±3FGL J0654.5+0926@i›``þG™@é‹@•À9ÁÃèø|~À;]²_c<æ?ÔS~"|ñ@þP
.'@S©"Ð\¿à"Câ¶v¨¿ê-ûL&¿êÝQõk&•¿ïÿcÚ½GÁAGNbcu?îuÚ­Ô‹?£±NÄ?ŽûY0¬?'3Ѥ­-? ã~ÞëÜT?ž¤°=Ñ!?âßÜ¢ÛÙS?Ì`IV?¸×iö<ïG?³Å}20ö0?Ô
l<¹‰?Èø¸H8â}?êZ—›0.?©(Míµ¯è?´ÞÚöÖà^?ž!tôþ#E?¸Lh0_ž,? Y'ièâF?âVÐ!
Ö$?¶OâdØA?ŋ}–F7ä?³h·Y‡Íº?Ќ òÇ7Å?²Ò@
¼Žß3FGL J0656.2-0323@kÊ¿ÞñßÆ£'À8NAûMØÀ:Óïµ/!V?ûÇwB¬¢á@ö{ÐÛÐ@lj
µ¼¿Þ…!vŒ6¿æÔ<k§T)¿åQÇ™8e¿í²ðF"QAGNfsrq?ì˲ýv?ºÚOI?¤þÍq[¢n?¨¤y
?´ªA9ºC?¶‰Â]ú+w?ÀŠ¡X
tË?É/+²`?¨ËœÆ'#ˆ?®}ÙÏwÌ?êPÝš0•?Éá5Fg"a?æWp½&0?²›låÝ[»?À=ŠÞÞI?¤Š
7'¯«?Æd´Æþˆö?®¢ áôu?é-¶?Æö?¶±(™?¦Q͎(H?¦¥MÁT*º?Å´áZ?³kcMúA3FGL J0656.4+4232@eÀâ€'،@2жâ—À9¤ÛÍÐfÀ;Ÿ<zڑ±¿¨›æûÍr@=¹±¼ûô@œ3`ª¶¿áÔÒKfÜ¿èäbÉ+‹¿Éß´à5Ï	¿äúµÝ`ÝAGNbll?î\È¢¶tù?¨Ÿæ*—³?g°è)ó?fÂç)=i?¨¸gTf8?¨#ƒŽ]ì?ïMÎQ‹?"S3š˜'?€ÔÒ;5?›s±<?‹¸MíZÂ?'$Ä^E´?î=çcçØk?—öÅ`K?w"êna¶?}¥>yÚ³?¤Ã¨†æàÞ?'ÐD(),?íÖƒä;?žnúX$Ã?i@¦-'?mLðóq)Â?°‡Km㬹?h?<µó3FGL J0658.3-5832@pË¿ƒ8.À6…rÀ:cþtŖÀ;×~ßÙïË¿ûa
Œ±@`Ï«¤^@7(`Ff¿ëM:£óm¿ÎK6Ù ¿ë÷"Èú&Å¿Ô;aSñ³{AGNbcu?ïšÜCÉ?mjºÔR?…'ˆ@ˆ•?Û|;Ið?avßÖÍ?fšŸ7æé?懲À†_*?õÅfîj'?`NiýÍ?tZ	]w#?Iu_#Âo?…«[ÚºG?í'Ýf@?™öÄÎv˾?Ÿ(¥èÿ'Ø?/j›ì?§=ÖªÌ55?"BdK@ª?ïB'õÊ?'%8C]©©?7 l´Ô¸$?Eu'Ò͂C?ˆkõ›çì?éx¬Á"^3FGL J0658.6+0636@iûg_ö	Ý@_ú D®†À9¤Ï©öÞïÀ;Y#)гâ¿ÝËY'¡@ãA¯¢Åg@ØeêV ¿èí¯½¿¶¿âî`<Î	¿çq¥õ¢"¿Ý'ô)¢AGNbcu?í3€ÑC÷h?±´\g? côŽNÝ?Ÿk°gè?¬cþ]q¬h?®†?äè,u?èá]PC*?ʀf¥õ«Ù?~q Ä?š0;¿pL?ÊjÊÈ¿@?É,&}vÔ?ë"Ǹ¶OÀ?§;ÄÖ_ÑÑ?¥fAêŽá&?Ò`V;?¹&¡Ei?£®2KÈ?횘Ío•?¢¤éð¼·?t'OŸ—U?vºÛ×Ý°?¶(̉à?¢Ontü33FGL J0659.5+1414@i"‰€²B@ oNó[À8I?>Ú0cÀ;_ÆÞ?ÿä+mìí@ëäj"^@
ùٕˆ¿äÛUiú¿ìZi}že¿ì­Tcuv¿ï5IçÙ"PSRPSR?µnUz"Ô?¹§`Žèàá?ÝUÔóXÈ?Ô=ì''i?ÝN•Ë"?Õ¼7«?"ÓLû§˜?·Q?…9y?ꚭBÄè?É/½5ËÓ?ÃâùP?Åý–ê?Öõ§"TÙ?°€…"ÔÀ£?ۉ‰w©ÉÊ?²ÕåÇ®+×?ËžÌu½?«Þª¯õ¿?€I½Ý§?'ãOwãÏ?îÑü8ø°(?¤×½Á;?½m<G?¢Z²H6ç3FGL J0700.0+1709@hÏ_¿ƒ8.@#. ÿê[~À9O7¢KðÀ;}x–ê'°?îÕÇOèÔ@8Ej˜O@Ÿ 䨿刻®tü¿ê"m/¥¬¿å
îޚž¿ïÿœ¹šÒAGNbcu?í­¶G.î'?±84ç‰dp?ŸTõ£Î%"? žVWfç³?¥z »*
Á?§ñ+âç6™?Û֞§–³(?Ê8_U³/ï?ÓÑþÀ³?Âë7t
ùù?ÐWcTbŒ%?ÇOÑ"šÈ‹?êY‡¢J"?¬@	ƒÊÛ?º8§gë??£«Huèè?²û†«€%?œ
©›‡z²?àà—Pz?µEnÐd‹?Ó³Dyui?µÈ‡˜+é±?È1_@¯ÓH?±ÁK蒑?3FGL J0700.2+1304@iFÜ¿ôw6@kóæAÀ:6±n¢u
À;œÃT~–?ù?å{Íß@Bs`õ¹*?üഀz¹°¿ïÿ¦´	\u?ïþî j¿Î¿âhµw+ì©¿Ü2qÞrDAGNbcu?ïàGNvQê?i›zÙ¶?LfÝF'WÍ?OÉT1ʶ?hžú8
ÿ?eJ½bþŒ?ë!IQ»–?ÃÚWµa?¦Û&ñ1n?¬‹m="œó?¼b´yŠ—?¿²_mB{ç?îWôUÏõ?•"5'Â?ŒwAcë/?|:1ÑeìS?£r*êJÇ?'XŽÈ4¯?ê8™ÜÌú?ºÒmí¿?Âúõ÷¥?º½¹kæ^?¤v[Qȃ?¡ˆ1#·' 3FGL J0700.3-6310@q`4óþÀ7	õ`iÍ#À:nߋrÀ;é}ü…!?ÖIÀ'*€÷@pL'8?ÿåÎÿ'r¿ìÃû"­Ãê¿ÎOÀêb×2¿Ô@¿©´Õñ¿çb=üAGNbcu?ïø¢2bK?K+èõº?;Þo'm|?Cûp|½8??O~òÁ??Gû}@r?ïsy•°
?Ž²TÆõl¥?lwg?lðO™žð#?Œ7M7Ÿ%?Š¬?O	>?ï=Ɲ?…pÛÛ>!?ƒ×¾ítc"?zvür?Œ¶½Mä9M?{p«'Ï?ï]â;Í»?‡·ãéËþ?c3ÀÀ½?`W7iÈD?'ü£20°?†DðÎSã3FGL J0700.6-6610@qL>_·¼À7¿F uÁMÀ8Á¯bYÀ;"–ÇWB?òâz뮏@ìéÄTXG@ˆì |··¿×zFm!Áq¿â.ƒç^Q"¿áˆYeµ¿åôbèØqAGNbll?ïåVÅ)ž?kØVÚy/¬?Fó¬ ä–¼?J]2%Àì…?dìO®(Ç*?hÌ\€K6—?ï]Ä»? §="y'H?€B{õÑçe?¸êû?—Ü`™^tá?œv˜ú° ?íOq!퐝?¢¿7":xs?F»Ð¸|ú?'†ÙsÆÚ­?¬eøÊ·º?›ÆýKÆ×(?ë-™A]Ü?°SppiÐ?•~Q|?<Ɩ^!Æ?À©+8(f?°
JéXhk3FGL J0701.4-4634@p®ŸðË°À1»yß¿î˜À8®àŸ°4À;aš>G?ö—b˜ì@wëb<á@''afÍ?¿âDuÖ¤o"¿äH†¿éuE£'¿¿ïÿ‹TÌ#ôAGNfsrq?ïžÞצ
¸?ŠÓF1›?''P#b?‡EðvŸ²)?h"¬ ±º›?g±½NOZ?ï­£|ëfz?‡8¾¬Ryï?]5¤óÞø?eLžÏ‡L?€ðl&ª'H?"1½Ç°?êœõ;ñ††?ª¹ýMï0Ð?¿`%Ks;î?¦SB+%;C?§paªº?•Œ1Å H?ï¬Ó\s?†¿»šù…J?Xð¢É,+¨?g"9Œ:P?Ýjr]¸?…T•J懟3FGL J0702.7-1952@lþ"Àh¡À#j ñÀ9aLF)¯ýÀ;Cä6uÝÓ?ÔcÍ,̚V@…©Îðéb@€ã?ëÓ¿å°p#¿ÐBÜtœ¿à~8iE`¿çb,žª¶´AGNbll?ïNí#ƒ?"?¬°ãÐ?leõp)…?mÝ÷E¨G?'•ž›
v?'ǃWE'[?ê;`bwý?Åø§}ø?›¼¢n«<W?£	)=±F?Ü&0 ¸}?ÃÆÛvba?î| <Sِ?"dœJn?'ãDZ§Â´?†>A'íì1?˜´ÝX?‹®ó0X?n?í'¼6×è?'ç|è{ä?…§uz	J|?{ý<ÿŠ¹U?´
/šŸr?œºcy°å33FGL J0703.4-3914@o;¶m
JÀ-;@Î&iÀ9›Wò/\åÀ;˜ôs®N?ð¹$y\@hó
¤×@M®€0'î¿Þqèa¿äphÈÁ¿ä­™<Ý¿êÂx‹%AGNbcu?éèHQ¥(G?½KçyïVÑ?Ár¿]>üo?ºµ3œrãÇ?«°}p±‰×?£{}d[!Û?ìVwŒÎŽ?¸×š±åk?§ªT'"IL?¦h§/̯?±yùúÏfç?±\{Ûáó?é0Sâ68?±|¿ÉÃö(?Â<_Ýø0a?«×øœ·lJ?²í½¤ýí'?š¨¯Yù?é#²bƎ?©å›¥wù~?¶«m«æ,?ž+ˆ¼†"?Àgbžò²?¦"ö3FGL J0706.1-4849@p4Ó_ôöÀ1ËóÀVœÅÀ9ob–PÀ;rd­(—?¨	,eÃç@qHA¸1@K¹ÆÄË¿Ý°¨vM±†¿çÖ?#P'¿ä¡‹^ $k¿çzÌìF(AGNbcu?îïM¹Çn«?ž;}º´C?†%uџ?‹&¤K/?—Ž;©[?˜LϤkR?ïIX<˜? øH?~W?{¶vÆpò?zy䖺èƒ?–É7zæÐË?œ²>ž_,?햳&)Œ?žîqɹé—?›"Õ½Qh?‹Å‰Tâ?¨Êã¾Ý¾‰?•¢ÆŸa?ì.ŸLÛø–?Ÿåï}m?ß[ýØÍ*?t7~¥@óG?¼Oe!¦?žˆfÏ"ƃ3FGL J0706.5+3744@fo•_x5œ@2ý¾?kOÚÀ9ºgozâÀ;Zˆ
%ð¿òےîÔ @ùó×'ĕ?þ= }Îã¿Øü½¦û=4¿ß£îX_¿àc§wÜ8¿Ñ-3FuҌAGNbll?ï§K$¥(X?žÛ¤Ã.ýj?jž+'??m÷/ðÁ?%—¬@_?žxddQž~?ï­éìš0>?Š}·ÛJ'?gukØnï?mÇ_õ?}PSÆ°i?†>Fµü:?íäJ'¬ª˜?™¶Œp¢`?š^µ~¿f?$pbÕÒó?¤‹ýÕÉß?'ú©§t­?îý"B@éG?"H;ÌQ§º?1"'"®…°?9ÄşÚÊì? vÖè?"%D…f"3FGL J0707.0+7741@a¦°)(@;H¡€èTÀ8監À;—³%]?èð¬Q}l@ø×è3Û@k_\1¿àd€Ý't¿ß÷ÿ`GéN¿ÞÎö ˆ¿åÆ9¤€AAGNbll?ïõÍYQ~ž?JeÑÐlM¹?9­›Y½b?1Z±¬=1Ó?KôìX©è?G$y/¦)?ï·("N?« ÒD˜?p1Ë"r0?o㊠*°·?t9ë6‰øŠ?vò¸ò%Ù
?ïg ªò[?€­Uû3?{ä*"³ì¼?sæÐ߉Z?ˆEÀh©s[?w}2†¸'k?6•wW?…Õ¬ŽE?]6j\\[?YVrˆÄ•?ˆ*o
Vž™?">Ûñ¿J33FGL J0707.2+6101@chy?ò^W@9a°,XÀ:aÆÄuÀ;ú'ÌÍ£Œ¿Ü+¹†ã­@`B_A@o Ÿ1ß¿çH©`['¿êB;ԗqv¿áEC#XØ¿ïÿ¤TÕç AGNbll?ïîÔrÕÊ«?jÿú¾áô?8fðŒ°«×?<¿z¢Rå–?\=^1>J?i¤Écur>?îÕqñ'ÿï? Nž×Ž?"ÕP'm
ä?'¢""¤?'|qK2÷W?"èډó›ú?îxCœ‰ï…?"NÃåBì?•"–Šñ?ƒÅ1¨º°{?›ÕŠh+"P?Œ«ý×5Ð?î~^×´5 ?½R?Ç\è?‰ŸÜõ
ÇP?‡[M¬ø"Ö?¡²Gy<F?˜?[ÉBí3FGL J0708.9+2239@hHtÿ†]}@+•³rì‡À9ñÅíhNÀ;²$€€Ä?áo'èƒP@$Êû¼Nz@œ¬_nû`¿"C2jòxi¿à'–6Hø~¿Üa=Yt1ø¿éR6u Ø,AGNbcu?îISv•ƒ?³Ðì‹aß?œfö²>R?¤E!-åRü?šÀ*6©ñi?§Ë؋FÔ­?íæ܋ý|†?¯¨Æ"°ó?XÞøc¿?ˆPª"·?©ŠÐ¬Õ?­XìiuÖ?íuž]íœ:?££™r,Ñ?¦
µRHˆ?›zh2é—J?¢™kÓóÔ?•L–²Àe?í£Áû§Xë?žELŽRó?"¶9?M?ƒŸïª@?¬4…Bmя?œ Öá¿{3FGL J0709.7-0256@k4œÆø@ß
ÿÇöÏÀ8JoÛZ.JÀ;³¦‹¤?ÜM$ñ|²@õ(‹k@‰û Iáö¿àÌTw%¦X¿çŒðw]ê¿á5pËL͗¿ç+óÀÎßAGNbll?ïį¸¥§‰?zåܗ÷Ó?HAmŽ…2?Es®a8À¢?z¦[zj?z'¦‹p?î:¢>#a†?µVÞÜ£àR?g6y+lîE?v%›Yù_?ªât‹Î?´Î¬vüÆé?íZÑqe"7?Œ©üN?"¾níjÑ?‡rwáÌö?°9ع™?˜v(—Ó×?ï‰>ù/"?…ü^ó`ï\?-ªƒD«'›?2¼çëB‹ú?9Ñ4¡rY?…Õ{ÖӖ3FGL J0710.3+5908@c¬|àü.º@9h~_o×À9ržJßÀ;ljÌ&´ ?Àæºòã?‰@ŽfÇ4?ú"—!U<¿ãÌÂó	¿Þ1ãAÙ>J¿ØK«"ÛÙI¿"r¦›N"AGNbll?ïéQš¢_?c
Y^K4?I–< @+"?D^ƒkZ?`Il=M•!?`ðz†vÉ?ïÈߘ
Ø?'þÑ#£k[?dãHæá l?lJ¿§@¶?q,‹ÀˆD¡?|pæWf>ú?ïÅ.#ѝ?ˆÔüÕcñÔ?…h	™+?}åê.O'?'sU­¹?K?g¾iR?ïqíàvœ?ˆ3ý$@ò?4õ1ƒ38!?J(Òð{.ø?'no+€ ?ˆ!?Œú…3FGL J0710.5+4732@e8·€4mÆ@6¹Z`ž¦IÀ9mM!À;ÅÉTrH?àÊö8ßx)@ùcãÔP@.0¿æ_p¿åÙLJœ¸¿èR¶ú0:ä¿èhn±í'¿íaœÊrøAGNbll?ïõ¯æ$?Q7Tq«ƒ?I@_
-?HŠ‰wp=õ?@I,áe™?A‰¿ZGñ?ïSæéó?j&&#	?†¥Ù¼Á´‡?'fªú?"`¡HÁ…O?†»o:~Ê?ï 5ŒG"?Š­3cª´'?ŽåO^,?ƒ"Í£VØ?‰ÝMMí¼×?{#¾wš'Ó?î1ΰß9Ö? q·º©šÖ?—]^	môG?‹Ú†Bq?¡4eíUh†?›âf7Ó
3FGL J0712.2-6436@q7µ ÝDÀ6*Ð`Ö­À: ²÷8±!À;ÀÀ//˜t¿ûpœ 4=t@£×‹Ê@î¤ûÍ¿Þ{&ëø¿áŠ¡EZ¿æÀ'30ë¿ïÿ§9.8¼AGNbcu?íÔ{uý©Ó?¯ü(8WQZ?¤ÛÜíŒÉù?ªc+'
ó®?›¸×e11Ÿ?›•¯Ý0O?ï*ik;@j?¢vŒ ?{£!¿§«‡?'_DˆtÖþ?"Ê
(®í?š^6{À?êJ!ñ$l?¦Ò±ÜJó|?¼DmìéÃ?£AÏû3<X?±jŠaòÝ?–Ð󾃾Ù?_9ØY?›Œºgê ?lŽB2Êø×?€sÀÔ¬Nß?¢=µé5Êî?™bA¥1t3FGL J0712.6+5033@dÖN wm@7Ûß 'áÀ8èpwa`mÀ;‰þÚf"¿Á<¹Ä²L@F›'{@ºÿÅÈw¿à¯âFdF¿ãE4oØ!¿ßÐñ­Šoä¿âa°¤ÊAGNbll?ïùuFSߥ?Eé–`e׬?%\Øçol?!'>
ì3€?DÓáúG‹?D/½þã0?ï·¿Y|þb?€Ÿã‰Égç?jó¨I=Wñ?kοL•v?v¦â"¸?zk
c5ô1?ïQÃŐÍ?†öA·Ô*?z‹ÒÄ8°>?uòr%H{?Žtå¬t?ƒ'7,ëÅ­?ïi"±ßÂ?Š4î$-'?I]7ü?HЉÆM\×?'À't&×?‰çÆTþ»3FGL J0713.9+1933@hµ«`kz¢@+/¨þ'j÷À8EìòÝÎÀ;=xmži?÷/Oxä@]‰2C@é¨Ì'jP¿Ü	E"¿å]Xë? ¿åð9cy¿èÓ~XHAGNfsrq@?ïÐ3M³ï?™{ñ\R7?a
Ñ=ãU?a0ÀΘ¦?n±¤zÓ"?™]b²%?^Tß?"/'ü
G…?baëý2|?iNmŸU²o?‡;æ/Èò§?'ªžŽÂÃ?îJñ ¡.?™?0ñPoh?˜™é˜3q?q)8Ωâ?žó£¸ZÊ?'EKsK›?ïç'&·‡&?pðö_¬?	Z@ª?*ßZ©ucc?g†ŽxVÕ?oÅA"Vô3FGL J0718.7-4319@oݝ`˜À+Iä ()À8L· "À:ó>FŒ¬K?óL"=@
 wŒSŠí?ýÜ<ŒAí¿Ñ]n€;N¶¿ØÀ¸æÕ¦T¿Øo'§9À¿Þ7F¢?ŸAAGNbll?Ü£ß7)j?ÈÕȝ?°w§æùg?«¥ny»d'?ß>XÞÜ× ?ÉÖ¨ü!?âTs¤ÝÄj?ÐŲn?ÐqW€ç%C?Çüê	°4?Å˂jº£Ï?Àó%\%FF?ã±KiB˜?³´¥õgIF?À¢§? ê?¥®øŸ·?ÐLYñê[?±R̍"Ô?Ñö%™ÛY?¶˜NI£^w?Çqçöì?ÀÜÇ­N?á(sø1?À_:wÕ_3FGL J0719.3+3307@g!A?ÐÐh@3Ú¡–'õÀ7•æLГÀ:õ-Iå&`?ù÷ë|eV@i1kÝɟ?ÿº*áU¿Þ=eÊå
¿âdàé©Q¿ãŸ.×·j¿åqî—YAGNfsrq?ïïÁÊ<8?[`Æ/
ú?G}¬…¹Ñ?HY%gÀçh?Tñ¬ñD´¹?UgÛéSæ?ïÓ@"3-Œ?z¸X'¤À?bDW˜"Ø›?f÷ûk
Ó±?j{†4M›h?tCC¿ˆáü?í½,ß^Þ?¡YW7ê?¢Ü•(Yç?˜³ïï€o?¡PœáÅÛ?"Ɇ|6K ?ïˤ¦2š?_uØ
0š?'׿Þ=Û?3‹¯¢Î[¼?ynîçÀÏ-?]âRW3FGL J0720.0-4010@oƒT`ªdÃÀ(/&Ɖ½À9à¾H¥‹?À;~áxU|3¿Ñ—=7²¸"@l@ÓVq_i¿è^
¾Å¿æáÐæÊû¿ÑžÀ€ÊQ¿ëUS€I€@AGNbcu?í…ÝÛÞ?µs sPZ!?[\Ï]º¥?ƒÿFû¯­?±¥¥#±È?´umpÌÜ?ìõÙBOúÊ?µ}_'ÙB?—:üAC–ó?™`Áÿ[ô?²'vÝ/Cò?±™ ¢›¿Œ?ëU7¦AJ?¨é .UY6?ª¸Mho¡?"÷ZRå	?·ú7¨'½ß?£nÃÔN³ÿ?ën¬oyº?­Ö™8ìÿ?y2ºŒÄž?yGlŠk?Á|¬¬GNó?­žºzсØ3FGL J0721.4+0404@j–À_k b@!¼@µpÀ97-m "ËÀ;tù»B`Î?à—Ô¹¼`@þeÿ¹3=@:Þ ‰ÍÊ¿ä
ˆ&ªŽ´¿çˆ¬1 ßI¿è_=Ÿ¸4¿ä-²B£AGNfsrq?ïÝW÷ø?qÒ»;F7U?IÁÃîd‡Ç?MKå8"c?l7—ñn̕?pœð"O
?î'ë'â(?§*i:°ÂÞ?ralnËö?tíÏ0ªn?¤­õD
?¦In<ê"Ú?î'#†M‰|?"åTh'+?"±œ•UV?t"»ÇÊò¬?¡±`•BÉ?'ÁLpÓ~?ï5*JàµV?vלÔÒþ?bYnZ.0ó?b–㸋?—ˆØ£B?c¸Ëª3FGL J0721.9+7120@aÿXÿu–…@<ú€d>nÀ6F#ÿ¹‰#À:XG·N¶F?öˆö#2_#@¥É}·ç?ÿ]g1<û¿ÝX¹ÄK7ѿኸÙáïZ¿à»~úÃr¿ã§LºAGNBLL?ïåí!ª?oÚÿ¾å >?;±ÃýU?A+B$™ô›?g~'÷¥Ö®?n<¿Ë‡É?ïÒBFQÄ?yrÞ)B?a]õ­q|?fm¨¥{*D?l‡È=;?sÚ}ƒ?ì5ÅۅÎ?ªGXÁyõ°?–žSf&…5?'»]áqx?¸ª<JGíá?§w«1CN?ïë¼]sª9?p_Ð"df>ú"¡,ÜN¦? Êá‡m"?d™Iüå?p[ƒÚiöä3FGL J0723.2-0728@kæù€õ]æ@Á¶@™MCÀ:Z`·Ð¼FÀ;‹Õ`EK¿ìKÈÀE!j@
	†Nc:b?üÅnA&:ý¿ïX9$câ~?ÃEϯ¢'Ý?´ÿ‹ïj¿Ðï‰ôÆïAGNbcu?ïòTÁ¡W?`š‹g5O"?2eøڸÁ?9ÁðÝÃ?V½Ïv?]m.zýl«?íó_)ÆÀú?ÀbõƒN"?t–0¯
2?™åèvô?®Hú~Ç?½ÇMÑ?î!t‹†,?–¡6òd!?‹¥% '*ß?{Á´Ë{"?¦ý¯O#Rž?"HÁ»–?ï®,ÿoÖ?'*Ù*¶Ð?FÜøiÉ?çϲh?"]¥ô‡?'IDÚ$3FGL J0723.7+2050@h­O d#–@03ËÿGs\À:Ղ}ô"À;³ÌQ|ÊV?¶ê#A@ËÞ/ ¬ˆ@3i~J‰¿å8'ŽT¹¿ì2ôG"¿ÆàÊv—r3¿ã䂳E‰™AGNbcu?ïÈ]"gßF?WÁ"rxP?:(Yq;"?=7¬Ã(V"?z.°4ü¤N?7®6e ù?ïƒëejõ'?–[Ñ@j?qtu7¥ö?tÅ*@­?†zìj¦È&?"¾:óÏâ?îõ›X‰È$?ŽáŠÙXoÍ?~|Ö˜2?r&Ÿåå0?™­Žy?U>?ŠŽ'V1?ïw?ސN?'#šÁÄ?N½Y$µc»?UÿV¶Æf?û-;K ?Í¨¦.×Ú3FGL J0724.1+2857@g² ìt2@3[½ ‡_À9¤LˆnÎëÀ;ÄŸþ7©¿îíPzì°@kDDž:@Ác `Ș¿çíí¸nŠ¼¿æu"—™[©¿äßOᔯû¿ïÿï-mnAGNfsrq?ïõ°µb?j2¦üP?&Y°iy¶$?78ñéìúÁ?Rhˆž?hÑN08?ï¶Ò8U¢õ?'öÎS:´°?f<ºÝHdu?j—5e'©?yx†fŠR?€/ÖR*?î˜ê´.Å?šëšÁ¦"?'c PBÁ?PB dá–?š¤Ù××?•KHÏϗ®?ïËB±~Éd?vÕå°üo?=sŠ˜\?JîÖËk£?x•Ib¥X?v$CoüÕw3FGL J0725.2+1425@itXf€@+Õà0VàÀ7Z)¤>8JÀ:æWS£ì?ø|§ÎÕ@9ðh2n@ø45f¿'¿á,H›Ó¿ãàNŒ€–¿äXɒ°œ@¿åµØ[4AGNFSRQ?ïÑaLÏb?¨bGÈG?gš£äÛW¹?r¾*¡i?…äþ³•Q§?¦‹TÿnÍ?ï®´ñ0­ý?ŒpÅÄا¥?^€,±W̄?då;>¦är?€'¾©‡[?‰½á["»?îG<7àŠ4?œXºáúE'?œt
‰=Ô?•+¯¢Žò?š¤kzÝ{‹?¬ÀVÚÁy?ïúˆ<PL¹?U'&ÇÂiõ>ä&ç¬Ö???Ú|h|?EŽs ä?U€@LaÆ3FGL J0725.8-0054@k69Àëíú@òÆÖ¤èÀ9EG1í¹À;kÛ._"?»ÍÌçyÌJ@%–¸Öq@'-ÈÈ0¿ä(›	—j¿äŠÔ˯ýo¿Ù+²ÔÍ]¿âr»7½ËAAGNbcu?îG†Ô?©?¡Že"?n ÎÏO?hýz×Õb?©¤'æ,5±?¨œîŸ÷]?ë-‡øq?ÀäuÈԊ?'€wnËÒh?"vO'k™?Á£:òDÁ€?¿ûY}éC?ì™Pâˆ;\?¥ˆ‹Ö2µ?šö…Ž·
Ÿ?‡¯bW¥RY?´w׈a¬?¢35àØãº?ìyÈֆǻ?¡HT¯U)â?{˜'°Û?tûäŠøb?ºx0:	·?¡3›ïL3FGL J0726.6-4727@p6B 6mÀ,;ý!(n´À8Æ¡ëw²¿À;TwÓv4:?ðMó=yÞ@"rYä¢×@¶- t"§¿â¿:pœÔ¿æÃÅð˜7¿çù=TZ†¿îK7ÛRelAGNfsrq?ï—ÕVööÈ?…ÿp~Kg?|$ïéÜ?zêÍ ®6ú?wðdöš¿?vR"iï…?ì\¨_î?¹Á!©4Ç}?ª£¹
yh?«=¸ :×A?²{>6E.}?°,üîv?í'ûQò]/? vÞCS?¥oDúO¤?"|‡¬ÿ??¢aæÃÝj?'
ñEÜý?ç¸2L"æ?±Nøb'É?¹¾ Ÿ?¦Y5à™¹M?Ä@&~&=Ú?¯ÍŒã‰3FGL J0728.0+4828@e2;o@9ÍÕߛªÀ:‹"äþòºÀ;çú#G-¿ú›yhKÃÎ@ÒÍ`Æ@÷ýÀ4¸ï¿êÞÜKðÄN¿à§ê{ož¿ÝDTî™Ñ¿ê<ߕ:AGNbcu?ïpÜ'jV{?'ÙNQ#?"²ì¾Â?'ƒY1?^>eü‡L?`ˆT1y¥?ﲖgC¯?†< ª£Xl?oõ@‹æ'?rª0Aã'?vºD¾+µW?³â92Dž?ìñ¼T9Ãà?£"â
µX?©Æ™'h¦s?›)oiž€@?§¡"û"?•ÉñВ?ï¤n–ý?KWïc3?;•
‹"pM?FS´"!qÜ?†{î"-?ì/ä3FGL J0729.5-3127@n¢å>‰©Àŵ ÝDÀ9´I窞¥À;Q¸Æ…Šï¿ë=iöqi'@–'%†ø,@;µ¿j
»¿ãô§¾6-¿êˆØ‰C‹¿í
ÎÖü¿~ǁfûjMAGNbcu?ï¨jmÒ??"^-¤‹…,?g
@"a½?n8÷ê"ñ?€"ÔZÏ!¶?TÑR9I˜?í=ØâI?½_=dmñ?"½_šLJ?")|''.?³€E¤(?¹Ðâ椽?í|ß'ìý*?œcqÞëF?–ÿԁf?"c´ÄÃ?­)–ïz"?—£ÇDø†ä?ïEŽóÔ^?'ÀÀÈ(ó?!%wpGg?2š·œ{?—9Ã2¤æ'?'Àå¡Ç?3FGL J0729.7-1448@lÍòà\̊?øb½ßôò±À9¾hêÀ;[Sã¬ã?ÖeäJþè@ÜÕô=Ôø@\›`C™¿à±ùĞøK¿èÄxãáo¿ç¿ûö¹Ž¿×L¤•ÃPSRPSR?àœÕ¿ðÓ*?ÑÙª	zª?"eX¹È?žšâÈ¡?݅ž*œþ?Ñ ­è@?Í?È2¡¿ó>?Ëñóƒ_$'?¢"«Vˆ»?§O0M7S?èË
gw?̇lèä?èIÐ÷GpÇ?³I‹^QDñ?¥‰'Uݤ?™_¤E?ÉvWjôü?²D$МF…?ä
µ­{×?¾ÁØdñ>?–·–Þvª|?™½Ý]±®6?Ö7"o«?½ô'GE3FGL J0730.2-1141@lxl_9K{@	Ø_ÒùbÀ6b²<'ÎÀ:l)±ª1—?ø'{j×@m^ÒsTá@¸Æ§Þ¿áapD­üJ¿äǜԷ|Ù¿äç|×I±¿æ£#$a"AGNfsrq?î«]Ó½+²?¤j‰&{?bÉL•¼P'?`üœõQKl?¤úÑÛ?¤Uæò_?îÐ&=ÌÕ?³ܐa]?a ¹À1n?o¬B@s:2?¡ë‡7ož?²ç»\F§¸?é]^û¿ý‹?®W0Ý.?¨Z꧆?™$rÛ³
¼?ÄsÉg:èM?©–d2¤H?ï®Xu¸Lª?‹:ËC
?%›ÁÞ·`?=³Ì\Q?"s‹©Z(?‹4Àš£úê3FGL J0730.3+6720@b'ºKâ@<™åàš	+À:Xg`ai§À;þÓôß:Ž¿â<žüÚ܅@¤­'ÊÈf@ëø :G¥¿éÆB+ôz'¿äòíVkWοèˆ(»`å¿ïÿl³Ì9™AGNfsrq?ï¾@»\Ü?¬á¨—5	§?|7¯"¸Ù?¬'%p3ER?RŸÊùe?pOˆã§?ïÎW^¤Ö?›Ã)'« ?ù®UNs?"­-àü¸?ŠY
%¬-×? œ àæÞ?îµZmå ?˜Vӭ͟Â?ž—$øJŽ€?‹ŸQ?ýLm?žò/¹ø½–?'+hM½eŸ?îŒÆãµ`?œÚì+>x?"n²2mÕ?"/НËau?šøqˆ!ð?'Ô"Âõã3FGL J0730.5+3307@g;öÿ:Þ"@6e>‰©À9ù>
ÈÂÀ;̐"£¶¿îvº8—îk@2ˆá:˜@ïý |¢=?ÍØ¢òŽ0¿è䴲Ϡ'¿ßÆNdMBº¿ÓŒÓ
‡ #AGNbll?ï]Ág‰?—‰~'Ç?aÙ2A"?f"†/…çÄ?'±7ªÆî?• S>4Sg?ï°ÕÐG­ò?,hô ' ?h#ÿwˆ#?oÛ+˜¿9¯?{ƒ dû]?‡´g"šq}?î…SôŽ?'®õÿà†c?â{N™dF?€­zñCî?Ÿd^š!‹Y?‹x³£ïhš?ïn8§ŸCž?‰L4-Éš?-IBÀË?2"'ßë?'þXˆ?‰:[™'ª3FGL J0730.5-0537@kÍóFí$@C·À AÀ9ÃÁð8À;Šf¿àîð…†	@Ä:ø‰@Í쟥ø"¿æSñÜѧ¨¿ä´Ä16ž¿ÅÇ$%hA¿êèˆ±ò´AGNbcu?ê{¼`:Ù?À]õ:¤è?Ÿºßæ¢fS?›—¤"L1Å?Â…ªÇÎ?¾nbFV…?ìv–é¸z?¾+¼Ë"w?‡Ø(½pC?"­ÿYåÁŽ?¹PCš'ë­?¼¥"³UÆQ?ë;¼Oµ
?«ÆF•^Ù?±.†b³é&?PAýT?´ó™ZÎnu?¢tt™NÙ?î=ü'E[? r¼½?`"Á¶d?f0û¯3?®2î城×? ;Î¥ˆî3FGL J0730.5-6606@qZhŸÆÚEÀ4Õ  0øÀ9ÑwÛðuÀ;‡±ñ\Ï¿ï;¹ñöw@
»7
³Fê?ü 4á368¿éÇO á¿Ø´–×ꯃ¿Á! ]FñÆ¿Ý8úÉpˆAGNbcu?ïҘ;%Às?y²¡Ox?J›ñ-±N3?OÈSú+)€?s`dGi?wØ72Ùf›?﹒7Xˆ?€·q&7?XÁ*~S¹b?`ZRq«ßi?}™Þ¾Í›?~GÓN÷|?î•)R€â§?'êðdҎ?ˆ•ð}?w€ÔòZ`? ˆ&•,Ya?ŒÂob¹ì?ïK65ï4?‰Ä
Žžed?ï7–´þq?ügýÇ?–ƒJ
ˆd[?‰º
£ë!3FGL J0732.2-4638@p0Ã?…Q
À)ÌG¢'vÀ9e¾/áoÀ;làæ_E
?úÜÐ*zR@šWÍ|2@)ë‰%ƒ¿Ø8qÂKOÆ¿æ¶É ûì(¿îýØP
´t¿ïýïmqٝAGNbcu?ï<e¤Úœ8?¡gЕ{?‹XV¯Šg?—šwï4f?…Ž@Jg™?'ã?b×ÊK?é$+)ä¶?ÆüŸwã?º‡j6Š?½T¾øº Þ?¼W9zLÄ?º+Yù?åC<ì¹?µR<dó3s?È}¥Ù"8?®ÏûøÒ¼Á?Ã9L"*ç?¬ó^_¶?á\Q'`O?¾=æɐU?ÔßÅÉ#²€?Á{S]p ?ÁÏ'sÃ?´	:Î3FGL J0733.5+5153@dÀm ‹]@;Vš ¨4À:pÚ7›À;×5Ú­` ¿ÏÐqûxf@
dÈÚ#øX?ûÚß?ãýb"Rf?èòKÅXí¶¿ã¬[ñ"׿½7'lÃf‹AGNbcu?ïho™œËT?®nð"03ü?uòiäÖ?…aþ;Û=?ŠëãÛ)Ð?­Ïà²å	?ï¬?5MÌ?ŠÎå'/P?tV,Ûi"?'•í›ª…Û?uŠF,>Œb?,Òfr\ø?îy
Á[%m?'¢ñT>n.?˜WLùR?‹·¥ºóyÛ?˜‡)»NYC?"nºòà[h?ïK¸´Û4?"pm¼Ñ
?†ÄÙSô?ŒY²"#Z…?‡ 
¼ïÞë?ŒŒæmÁH3FGL J0733.8+5021@döè ÓI¿@;½°ŸpÀ9Å»{k±)À;Òîî_Č¿ñ§fiœ@îKAFò-@¾ÿ¯£¿çúÚâµû¿æª¢_)Êî¿çCÑ`&Ó¡¿ã-ËÏAGNfsrq?ïü~X-G?Br-aÌ?#˜VáôR¿?!7"ú!Ã?2Au›¨ç??`>5m0@?ïѤmÙÙ?w•Mö{?aA‹(<G?c—‰Ñ¼Ã?mZiê&Å?r!%"?ïŠ^,JY|?y;·./0P?pÆڏ¸Â?c§+ud?…ß!Ĭ?tóÖúTZ†?ïíH¦ìcÕ?a¬õ6µô¿>ÿ¦9Gÿ?>†P¯õ?bwÓÇ)œ?aT]õؙ3FGL J0733.8+4108@f7)à¤&@9
ohیÀ:.ήN\"À;ê‹y¢ƒ? ¨8t¹Ûñ@
(2F#Oæ@ÆÎ`u¶¿ì˜î
V'€¿Íɉ¬¿–¿áf`­G~ø¿×¶óËØõ¿AGNbll?ïÝQÙÎvÿ?ol\É1²&?\ZuàÌÍì?^Õþ6ãCI?d€ëA"™Š?f»ãÛZ?ï€âÌ?Öôڝ5™?~×E÷ˍ?ƒÁR™?€Ý'G?ƒró‡l?î¦ÆAN¾?é*^½s?Ü—Üè÷?'ýéãÅaí?š_ù?U?‡´½Îʶ?ï#fò›<ö?Ž)_îÝQÄ?|0ª0합?y8òÈ*y?"†÷ \ûÐ?‰…Çwí3FGL J0734.3-7709@rŽ¿ìºÀ8(àÉÙÓÀ8аô)2À;n`TÔn?é"tþžoÜ@H50cu@R'ıJ¿Õâ°)åù¿æHû*‹¿åðûDU¿çq$Ê(œpAGNbcu?ïô×vÀy?M›†Uâ?EÅßâ,?Bº3XéoN?FÝ
Ýå?BZýÊí='?pŠÎ?&à™‰0?gÀëpõ:?jXwùgºb?‰ã‡ÛÏ?‹Ý|·À–K?ît–¨Ž'e?"¦{Ôi—?"…'9k?‰Ù`ß>
Û?œèÔûù?‰Š'›±u^?î]Sàžô?Ÿö?FqÜ?sôÁÒ2£?qc`¦£?§¬)ÅoЪ?Ÿ:.	MŽ3FGL J0734.7-1558@mž@ÈG,@ž 'ðÙÀ7⥤i×4À:÷ì^òÕ@™ãC0×8@²ß¢<€d@"fx/º¿ÖÒXbËt¿ãAVÊŔ'¿è%n+¬¬¿íì¹®€PSRPSR?7€™¨ªZ?Aš¡±ÒSÐ?ïÇ
¶+C¥?'
n
=}?{OӇÂ?°a&*î˜?)ùºwUü?I«X
à"š?íAb'm?³ÕG"ãzI?µê—çi?³Ð½"Ëmj?™ËQô?Ž+Ë0IVC?ì_0ñ	²5?¢f7¿?¶Æ£q±U?žÉf4Ìøô?NDJ|fÄ?J3éyHX?ïPHXYs—?ø%EO¿‹?•Ôº}©õ?6"'wY3FGL J0738.1+1741@i;dÀßXÁ@2'ŸªTÓÀ7"^™éJ²À:ÅD1ˆ8H?äëWÒNí@yéØ÷'"@
?·¥ô¿Ü3†Ç¿áÏ-à8¿Þñë²7—"¿Ü»ã"$VAGNbll?ïì»Æ2o!?`÷Ià[[«?5Žïك"•?4ÈÕ[»r™?`'[Ò`z•?`	hú`?ï­£¿+Ó?";p
 ?k3…ë<›?míÃ'I?{â&Ýtwþ?€ÿJqO¡?î'[Muê?œ¼¡Á1•ã?~|ý"Âúú?|~öu>‰^?£
®X°Aô?šc_ìø ?í)|'õɳ?¥÷nÿÉÒ?d®Äë.F?g³²cÝi?¶¥ÈJXö?¥Ç‹
w3FGL J0739.4+0137@kËßÒc@&е~ÒmöÀ8%W¨]'À;T»ÉoJ;?û$G%Ž@>«6z@ SMÚÔL¿á𗳡"Ê¿è\·€à:=¿çËíSÕë¿ìÆ©C'ŒAGNfsrq?ï*ØðZg?™–£6?"èbu§¹?"ЪEß y?{Q‰±4Ž?ƒI¥9ûê€?îNàEß$?¬u'Q랔?‹ð2`ÿó?ÇÅ¢7ô²?¤Nÿ•v]¸?©Ä¬¢µ6x?ìŠEø\Z?¤m5¶tÑ?²"¹ô46? 
¢¿/ê‰?¢2,—QÎ,?"~Â6?íººÊû"À?«sj>±?š_Ÿnx•?™";fêŠ?§$ƒ™­?§uE'b´3FGL J0740.8+6621@b¶°À&Ì@=œzߚ.ëÀ:frû À<Àu¦uJ?õ»½ ´ëÛ@7[íçy¡@1Ø@žUÁ¿æ]¢ÿ/0Ö¿Ñ~"´Ç6O¿æ½"e¹ú¿ïÿïÝÚ!…PSRPSR?ؤh«m
ˆ?Î8dx]!?âÝ'½?ε"òß°ß?š"P׃Ç?´#[ܙD»?Ô
p{F?ƽ(څ²6?ãª
ûzû?ÆìÍ+Dz?²yçã*;?°Ü^\
±?Ûi¯J)ª?¹\Ú¤øÕ?ÞAGœVB?¸°ï¡ç·f?¹VÒÒÒJ?£&?×ÊCª}N0?¹ÔŸAè‹?ã:<œ*C?¹·F[RF?œ1ÒèT›?–dèzð1Œ3FGL J0742.4-8133c@r]…À3aVÀ8ù_{šÀ:ÃÃX¯Ä~À;»‰'ä™r¿°º"ËZ…@	Ü=IaÕ?÷l?¸ý¿ì‡/ÆäwܿٓtvŸn›¿àÁM<ɵ?Ø2E-¹AGNbcu ?ïéÌႥÑ?egd-žd?3gØd­?8nÌßÓma?cÆ=bM®J?cý7T°('?æYׇ?™^mÖÄq?`cæJ–™?y"Ì~ݱ?…ÌÖäxV?"s'¸&÷d?Šçv~?" yE¨›?"P¬ŠOxå?,h?š]¢Á·I?ˆ8Æ¿]?ï?Ù{ÐÈ/?—´>Cú?8"Nwë?N¥#+
-?—¢¾D­.?—®î½5Äâ3FGL J0742.6+5444@dam¿‹›ª@=Œ`Ëò²À7ÅÐÂû'³À;3ÁÑÇ'?÷¿n2†@È8'ŸT@(ªªŽ—¿áV£Ðª'¿ãôIL
€É¿äŸ&ãæç"¿èU)ßÕòAGNfsrq?ïé·IŠA¡?e‹ºKÛÄ?[[_úèž?`«
ËDƒ?Qw‹Óð?T÷ à^U
?ïÔ@³óí?{úºH™;?`ã,gïÚ?eÁ†ÏI‹?jÜ …ýÔ?w¢¶¥NH?îý[•ˆÓù?"Æ煰É?'†înã£?Œ•øÿ%:t?›ÞÀí:Ê?"+·(Ö?ïý0ÿ7Ú±?I5×݊ÿ/>ÚJiv]b'>öúû"r?6ܛQß?I	´Wd
43FGL J0742.6-5623@pÍN wmÀ/c1àLÜRÀ9Ëú/ÜfžÀ;£'ð	è·?ãmÛç-1x@7º¢Rв@n[à¦sr¿èV€G솿âM.6c¿ïþœ ::¿îŒxϨ'AGNfsrq?ê
µ]ëß?Ã9Yë#Y?ÃÒKŽ¸EÏ?Âtôú²?™½«U?•¡Äæ#ÎÑ?êûXª?À(>>bT?²SI 2ÿ"?°3"5•?µÑñÄçú?´i_Rhµà?ë#˜qV½?¨«•±^š?¸EŠFôæQ?£3p®"TS?­;jëǓ?•]¸ œ%?äØÇ3?½"2ÕI¦?ÐÔJ(OD#?À%…—Ô ?¼~ßüµÝ?¬¥-gƒ3FGL J0742.7-2824@ny)Ÿ¡—ÀÎE s'•À8àa'ÑÖøÀ;!º+àX›?ö¯þr·,§@C1.ãÃ@íèô>׿Ò&'Z¶°¿äíî/ýW¿êàŧ‹í¿ïL3íÙPSRPSR?Àßøa—/ó?º °Ÿ¨X??çûTöÞc?Ä9šÁ3?¾eg…Þ‡y?¸,
:Ëíý?‡÷^+‹0é?"fmãކ?âHSš?ÇrÉqÇV;?Ú°(h}¡F?Ǥ%Íìµ?Ò¯—>®%2?³]¸¹ÞÝ-?à{Á! ?´Ð C=.ˆ?Ê<g"Ÿ1?ª8‰ØØÚ?ÁÝu{Y?£†YñŸ:?å±³?Èhe?¶ºd'÷?È,U‹cO?±<¯'͓Ì3FGL J0744.1-3804@oŒ-@ªêûÀçÆ«±ÊÀ9®œ­JP†À;@R,†q¿£Ì0ú&@
m‡Aþ'@q³?ˆ?¿ç¼d™Ì¿æÐ9Ó$C›¿ë3@ð=ÈÁ¿ïÿ+‰/OAGNbcu?ìÌ`õ?µ'Eê<T?–Ìë[":H?›z,3f
‡?³éÄQrc?²·4Ã-=5?ÙÆÑç;#Å?͜ÒÿÖ-	?Åßå¢"ñÞ?½ªº°'$?ÛI;G³cN?ÈæëV 8?é«")õJÓ?«;%B—Kl?µ2Õ[ÈY¦?œ×i¥¯ø!?½tTOÄ?¤8£A^žL?àÓ¥xʉ&?¸Œçq®z?ÄfÙ¥4a?¶hNÓ?Ô%H;Ðì?·*|¨×3FGL J0744.3+7434@aˆÏÃø@=–²ß»¼ÚÀ9Êìˆ3@À;Ô=ß^ŸÉ?ًž`Ë\@Ú6n&#U?ÿÉ¾Ð_Ô¿æ
ÂmDÉU¿è¿²sð‡¿Ñ]i4'пƧrŒ¤AGNbll?ïûÓË?$?>Û
ÿa5?UØáDB?†~H€?@µõчG¹?;ÃUÀ?ïÆSçƒNý?{mô|°>?gßeì»Ì?h†ÞM9á©?q‹b$0?u#L[&/Z?﨏‰Q»ë?y=GVCFå?fçð8iC?c€,PhoB?€"!v–?v1ˆ&?︮ãßî%?{&ŽLL0Å?,켔Ée?<>Ô»•?`"±Q?z±X¶qó3FGL J0744.8-4028@oÑÞß)À 	ÙÀ%I'À9cý!(n´À;RZ8Zº?åä68@
h/žÿ	5@·[à{€T¿èø-®d¿Õ^Ž1퟿äC†Änž2¿ïÿž'ƒ© AGNbcu?ÅüÅæÿ:¶?ÃTì¥éhµ?ærSÕ¤?Ê}žºÿºg?ÀpÌÝnº?¿VûlÉC?±õêøüт?µŠÜß¾Ú(?âwMÏ|,Ø?Çir­Ã®?֓é¢Èqñ?ÆbâÃ|WD?á5è÷Ô¬?´ã̐Þå©?Ó8.zW©?³švu½Æe?Ä·ÿ,‰þ?¦yyü9È]?Ðሃ%ºd?¶ÑӇ=¡I?àTa²
P?ÂP6b!%Ö?Ìëh1LUû?·	(éˉ®3FGL J0746.4+2540@hWFà!q@6Ø1ôoÀ9MC%¾=À;¨¤Ô`?¿ô¨cpŒ@üç¨eÝ@¶šà@œþ¿èÎíd?οêß"Œ"Dè¿çO¢D
 ¿ïÿû
LàAGNfsrq?ïþœÎˆ?.\Ñ>B"?i["ï?Ïïµ1/?$rxq­H?(ò¹¾÷?ïªg–(Ù?‰p×âÏŸ?l²lâ'‰?mßæÓº²7?|s@CÜm?†ŽcGou"?ï)€ù@?ŠÕÄU7ÙÙ?‹&?(jà?¬Š¥eF*?Ï—'‡"ø?ƒŸ´Ò΋—?ï|€ß?'[÷§ºŸ7?Qɳ"ä?ê?h9<í ˆ?ŽÆ)U£r¤?'áZ9Ð[O3FGL J0746.6-0706@l6Èó#@!½•`$À9þ!ã–¹À;kfKŽt?Õ:[¬ñ@ºÁeæcÍ@‡Â yÒ?ïìkü'ƒR¿å›Üc‡}§¿â÷ˆ"¢Ø¿êøÈ¥î(AGNbcu?îæ-'§?§eŠ¿Šï?}RF¦îê"?ŒÍ.Uò?›åÊd_Pã?¥?>Ó¶?êçYé¦?t?ÄÀß­Î>?–Jœ2ßÙÐ?˜/ÚÛeìz?Á™DÓö?Ã,¢Z+'?ê¯OÞ?_!?¬ :Òé:±?´ID 	ú`? #©–ƒ:t?¶<<íûš?¢î^Úz&?é§Ýýðœ?µÍܓ/>?¢ºàÆÝr?–{{q³àT?ÄÚPØL?´°\Mœ3FGL J0746.6-4756@pUÕ`"¥À&¢ù;.ªÀ8øžâ®¶aÀ;Wƒï
iu?æüEH3 k@x¡Ú±@¾_쥿ç®(&ÃA¿äãˬfOë¿á%]èÇî¿ÖM¹º1¦AGNbcu?ïK±Þ8/?™`ñÝA;?l*Ó#ÄmÜ?tXN¥æû?"iԁŽ»?–¯õ®}!J?ïû}-ãH?¢ÇD¥¾Ç)?tÁ'v?|U|zÁÓ?™ÛŸù¦˜? \ðÜ
?îR¥bÃà?–BWc>ôŠ?'u»£¿?'5BÎ?¢UJÌâX?'Gphýá~?í¸Çfpý?ã°†!Ÿ?møˆNy-¦?pb÷½}?±JŒÐ®ª?M3þ]/3FGL J0746.9+8511@`à·ö@<. Eð¥À:/(âwYÀ;ÐÍ×°VÀaK:»è¤@ïàÚñ?ü˜ì€Fac¿é™'Xßj3¿à&ÀøÇì¿Ö8ðÐÞg¿ÍÅaðA¶AGNbcu?ï腗mùI?"YÛÙ¢?5"Tµ§ž?5+	– ?dÖûT¡s?"EëÒ<mÒ?ïÑÏðÚý?xÞôK?bœ9ëó?dûz†'|m?lrëÖo?s;,3.Ã?ïIáSÍ
?'<X~«È?€Ý…äÕÚ-?sˆ¯è°V?Œª%Yöâš?xòŠó]‹_?ïÝ°*$?p1Â'p*>۝ºjñ‹>òXV½ôsA?q!Ð1Ú?pSA1U3FGL J0747.2-3311@o
•$ÝÀٟîó=À8ƒjƒ+™À:Ø G2Ä?Î,Ùx'ôö@S­|$"@y¹h¿â50hJ
¸¿æNíìW+¶¿å)‡ZID¿ä…R\Ä&5AGNbcu?ïx&Œ–Ûé?Šñ7,j¢.?^½6MA?^"®ÔQ?Ž¶¥ã?‰çÇ&e?îŸKÏ Ÿ?¯édžk-?s(Éôò?xòòRÂç?£«+mô·z?­Íô­3­?ëÒ[ý"ƒ?©§|ºZª?žšª¬—,?'=ð)…K/?¹Æuh¶!Š?¥4¾G˜Ç?îÍÀ!÷h?–þKá~ö…?>‡¤í'o–??‡Žè{'?¢æî¥Ud'?–éUgûƒC3FGL J0747.4+0904@jb`RP/@0ˆçÖyõÀ:d%‹ªÃŽÀ;àК·§?âˆéߓ_)@Hî=à¶9@‡Â?ÖØ¿ÛB¦¿X+K¿Ó $ØÒiš¿àø°ªF(ó¿ãðsÚ AGNbll?<Û\Ï?&?6,rr?|%U¹¸6n?ƒ—ÛĨa˜?zؙb?À·"¥?íAvBR|?µFèZLû?¥{ÀµðW¬?¤eüäÀ?¦sGåꀝ?®wÉ;®?îc*áPs%?"ŽNkÅ1?–‹íÅÛÑÛ?‰hAÙa¼œ?¶É{?‡5ȔkÕZ?ë9±Ëå6Ã?©¼ímÙY?´a¥ž[?¥}3'4×?±ÑXû8G'?ŸØ
ua3FGL J0748.0-1639@mF÷_²íþ@ÎÙãÀ9/Ã¹þ"À;CÖS^Kæ?õ–qÆì¹@ۖÛúT@Ö[ 9ÆË¿â
^¿èGCˆb\¿ì˸0F¨¿æ@ºr'(AGNbcu?ì!t"úË?·Ö®×´?©Ÿ©Ö†€?§ý_¡úà?²7l†læc?³QMf¢Ò«?ã㉂ܥ?ÎJ9šý4¶?±#E\ë¸?³‹Æ¤IŒD?Óñ¤(ïzê?É¡k*ä1?éí_?>Éx?­8ˆý|·w?µî™Y…·?¢Þ)¼?º¦l¬"£?¢Ë¾?a"?⟧b`FŽ?º"?3€¼¡?ËG¨—KYL?¿¦;¹­Ä?Ê9¹ß3Œ}?µO*X.é{3FGL J0748.3+2401@h'FŸ¸@6­?i¢[À9ÀÜ0À;³Ô&]aÛ¿ð ~ðËډ@[µàÏ8@@`k&¿àñðj¿ä,fꉏû¿áéñd '¿ÕÙ°"AGNfsrq?ïüÃ¤†;?4nnè°é?µ}5+ü
?7þ™wÊ_?835(ªR?3.Æ1G?ïÔ47qł?zE°{ðÌ?\ Sÿ*t?a—ænBW?m{¹d:èù?v"Šg?ï'ÿCR?|A¾Û±ÎÖ?sïpä"?k;;k¹E?…°·sø'?uÙcóeÉ?ïöbس±á?QK¤.ÈG>ÊKE¡òÛ>Ó±,¬"ñ?S-Brùlò?QHsR†®/3FGL J0748.5+7910@`ß2_c<æ@=GÐ@ÔÀ:›OC427À<)LqMJ?ñj®òÇ2Y@£àÒ¾(o@¿ï©H8?Ñõ%†wRó¿ãæZû#L`¿ç«Gþ‹$¦¿ïÿ¼rÙÞ¦AGNbcu?æácO̼"?Г"§0O?Ò/êg·"?Џ¯
롁?cºÿgº®?lÈ%˜Í~/?é.NðyA?ÁCÇâÁÐ?ÅZÓ½ú¤…?½Á»j–³ü?§´¬
ÙÛ?§.9óή?ætí¢Â…Å?¶ˆ~BþðÝ?ÌìÐùQ¿ì?³›îýŠ¢?²~ð÷HQþ?Ÿgà;›øg?ås¬DèCª?¿:|¹ =>?Ҋü
'?½½ªŸïl?¤tsщO?¡Œ22Ø´²3FGL J0748.8+4929@e$¯ÿ6¬d@=XlÿݛQÀ:3½äÒ}À;âÅû!?ևæ³þŸ®@
­ÍŸZ£»@¶jyÍv¿ÞíG€ù¿ã©;ˆAWŽ¿å¦ÐWN¿îÑzÎþ*hAGNbcu?ç^́Î[J?ÄkÔ|X?Ë, Ïà+?ÂË7•×ì?­`´¤ÖÊ©?ª‡é±qÀ?ê4;ó€õ?½tOÛÿ?ÁSÓdu4?·'î2Œ?§g¾°Jî?§'µ'Ã-?ê20?ª6°üˆ?¼fsŒ/?¤ÌV®=h?²ËÂïj?š¾Èyi³:?ènÐf€¸±?³uaÁhÿ?Äy¡Eeø0?°H»¼È:±?³–:A.J?£²·:|3FGL J0749.4+1059@j/
€CR@1˘<eâÀ:¬ÿiÀ;¿­Aí
?Ôpw%?C@™#îq¸)@ŸÈ_ÂX¿ç&J;¯Ðà¿Ý•tè—A¿ãVòì'Zõ¿áKâù×>AGNbcu?ïö2ÙK[?R'* tW?2&éÃDn§?/I(Ð[™B?N—¿¹0\Ô?Pë¢eÊHò?ï­´rWP?ƒ»O?l¶k+¢?lml&:pg?{랉aâ?€hŒÂ
g?ï}E:(Ä?~-I¾<E¹?{ˆ†'µ?sõ›‡8W?'÷kjõ
†?sµ4[«æ?ïLŸÅ0 ?†¸máú͸?gÚ(Óß5?c'»¤?"lâ?€"?…"Q*Ëá½3FGL J0750.6+1232@jì O*à@2»`c'À9c+Hƒ'À;pClfZ¨?ë
ªj³c@VF,	HS@J:Ÿäƒ¿ÛTÌÍ+J¿éX¿Ž˜+'¿âßã鰝¿è Ü/&šZAGNfsrq?ïñm1,®Ñ?\Ç-…¸É?;Úá+Ns?7
ÚÞñ>â?V.åfWŒc?ZlÊØ
µ?ï¯B»>
?"å$'å?n0>íù¥?o±á|%Ö?yf¿œiý'?›q""÷?îæo¥¼è?Í"v/ß?†û W,	á?}21äŒKü?—´N?²^?‡²Pw_y$?îÜ«à>1?˜Ý:–ß0?p5
Ý%?m®NP´ë? .žÁDû?—àp¢p3FGL J0751.2+1806@iX;o@5ÏÀ¢À9Ò»úÀ;¨•Š@`B@†äÇ@ïßq<X?ûxt=i—ô¿Ú"DPo¿ÓˏNÖÁ‡¿ã^;÷š¿ï!Õ2!oPSRPSR?xíöº),?vávv¯?ï¥þÕßÁ©?ƒNÞLø?tá§eY?v˜ÝÝKÙ?cRÿc¦Ó? Ì^µ{?î܆躏ç?©½Ÿ
²8S?›½yhü/½?¦Z•O,«Õ?¦¸á¼G·ã?™'qz"?ìžLñ?¡"ßãRS?¯eM¾é7?•$bƒ€ð?¨T‰ôÍÐ?—¡ÅC?í†ñGRýÅ? Ÿ4š6ª?žxÃ,²?"ï+¿æø3FGL J0753.1+5353@d†A¿½ð'@>…Á?ÐÐhÀ9?ª¹|ðÀ;¨"?…J¿ºÆ^;Ó|@ ®÷#ã@ØúÀP»¿Ñ•º'L¿ãþ-Äx.T¿á5(²7Œ¿ß_~þ°AGNbll?ïó6¶Å0?SN ®YÍí?1‹ë/vúV?*ß9r?U/—©áù?R ÃÚÐÃp?ïºí0¾?¦¿ª;{'?lLs؝†?l Ôüêü?tÌOà4qt?xøÂy½ý?ï6(¯àÒ?ˆB¶ñêϔ?'âÓÉÅ2®?z(]ñŸ«?">XI?¾ºÚö[?ïV Åþy¦?ŠÖÁ®Sjþ?Rz•ØWG?R&˜/£ñ?"=â«Z€?ŠpüÀýŸ¸3FGL J0754.4-1148@lÙ)¿*å@ y–ÿáL6À8¾2lcÖiÀ;CÉv7]?êÅÐsYN@—M·B÷Ì@á©`6 £¿Ø@)vý¿ãsQŒË¼¿ßMJ!G‰"¿âª¦žS¬iAGNbll?ên«CY?½F:§²?¢ò›l[º¶?ž~#r?Ã#j<ñ?º¨†4"%N?äÌ`¢©Ú?Êj	α?·×á_óù"?²-̨µÌË?ÐqFcÕ­ë?ÇpóªÁg?ê»ÜúÝßh?©@Kú€v?­‰œrGŽ?˜üá¡+?»\Ið`ù?£We—¹!Š?ãòI7ّ6?°t¼K<'r?¸8;Í(µ?©µ¿Åú¬Œ?Ò
^צ?°H
HU3FGL J0754.8+4824@eQ4 -œñ@>(l <K
À9š0˜N@À;ž"Ž½ž?À¬ÔOß!Ÿ@!eÁzß@$=ÿêÜW¿àêø2†K¿âÏØ°ZÑ2¿âTSK×nç¿ã»´0É¡tAGNbll?ïkѕ²xð?—²óPôÚ¦?p£a=
Ɲ?|%x¨šÿô?Œ¹éôÚàÓ?"§ð܋¶ß?ï9iq»Ôž?"YYë²û?ˆ©o'¹?^?…vcÝ0­?ˆü4iQ™?xŒYQk?î2 »ü'?š?P!Mô?"›*\#µ?†<¨‰ÜÀ¹?¢Þ€_%"?"pOß­o|?íчé¼O>?¢ …Ž7?Œ8¹hÆ×Þ?"òÏ>³(?«ÙS
	V+? 'Öi¤ç3FGL J0756.3-6433@qTR_ét£À1Â\ÀË6ËÀ9ޟð˯–À;³x«ˆ¤¿ÞtÁ' @atÇ},¦@¼T@(4¿ä"ôµ¸Î¿åM7È2"+¿ãW'Ñ_Ú¿Ù+Ҋ뚲AGNbcu?íÎm;'?±VlÜ4ƒn?\ö]-õè?[šŠòÉ`¤?±½µ¾¿®?±6Ì{"ò?ï•ùºcˆP?‹!(SR?aÄ
sÓÌ?dàôü¦;5?†ŽÊWwC?ˆÃY²Eß?íì)%ÌJþ?œ-3íyȁ?'¾*'F²?€/ôpu?¨^Xb9¬Ê?–²J©åÂø?îþ#^å<²?N"—z'??CU›Ÿ®¥J?Dªá2s‹+?Ÿ çFZô´?8¨À¦å3FGL J0757.0+0956@jiʞõ#-@39 4¾NÀ8"ÕϪ͟À;W4H)?ëÇ:
V´Ü@"Ë'Rz@trŸYÌû¿ãàN#Ïh¿ã£dÃüÆ¿ãq
â秿ã´^zù_AAGNbll?ïíÇ@¹r?^Må§-+??΍tÈë?Cîæ4'E?\}Û/éá"?YÍÃj¾óQ?ï˜)Z,ÄÕ?†Vv˜î0?tŽž_óéô?r™á;}Ú?\´‰©¬?€ñU析0?ï;›n"p?"½š%€?€rfaáý"?u²š>ÑÎ?S^þŽ3Y?Á3/b?îa•òqp÷?œv;ãê'?~ Âõº>?w]âJdI?¦" Š9G?œ(ú3FGL J0758.1+1130@j=ÒàãG@3õ[_¢'À:_Y²"ý[À;ÒNér?çMÒ%U@G®¡hšô@QFt›?à‹!Ω=H¿çM>Dð[¿Ò@bÒn]'¿ëJ¥mQ+AGNfsrq?îø—~ã°?¡Ë>ïDq×?Œˆ†[½Ýy?Ž·puU8?'¨Í"›,?›šá¸WÚ×?ìѯU&u?µÚ΃íìâ?­rêW!†€?«›§2Õ5?¥{곌6?¨49~ǎŒ?ë·{¾ø\ð?®ϽŠ(}?±×&á.=?¡D+A½Ÿ?±'Já[êC?£›É¡YÑ!?ê™9îTŒ}?³	èuN­Ë?®$E{&æ?¦¦Cš6mÒ?¼$
Ïț!?¬ì5#œUN3FGL J0758.7+3747@fÕø -à@<àu¿Ÿ½ À:—±æ—y.À;û>ß8à¿ÓX¹mR‰@sŽíï@>¥ 5"?ç‡ShTJ¿á'[ËF©¡¿ärÜDäá¿âÅz·pAGNrdg?ï뾤£°??eb…oj?VÉy=?[¹h²S5?Qôí­'(?\gëp:Ÿº?ï±åþêÏ¿?'$%P:?qm!Ææs?qÞW%"ë?uŸÞē9~?{¶¶Äm\?î຦B*?ŽÞ…eߘû?Ó0ˆö?…X†Ö¨Á?"›2¡?'LPÃ7èÚ?ïI®ÊRýí?'ž¨cÅ?iMÅChÇ?gnlsEØl?"™üü÷ÕU?´Y°ßxh3FGL J0758.9+2705@hI#ßm¹A@9òσ³~À9ù"'Ñÿ<À;ÓËwb7-?é]:êGî@†lQöÃ@ —пæýGÜb–ù¿Ùæ×Ê°¿Ü7£8Š¿ê驀'¾ÇAGNbll?éÚIҢћ?Ã$r³\cã?ÅÇ@Œ)†?©ÂsËÌ?–|ÁG¬€€?ž*Yw˜Þ?á²µùršÊ?ÇÝux2üg?ØÌbµn?Æaœ1Y6?±û©–¼?¯;w¶)Rö?êv?¤…?°*nwövL?¾GÜ÷<>g?©'+ª•±?±qŸ™w?œZN;Z?å)fU۞$?»G¶Œ"?Ï~'¹pš	?ºG
›Ë3?··©ÞAÚÖ?¦CH¾ÓC3FGL J0800.9+4401@eø6ŸÏ=À@>‰M߆ã´À9ë̗ó§,À;åáMQ?áÎn"w	¼@
dSÉ&@X?Ý»¿àJÄë	¬Z¿ãžK'gµ¶¿ã•ßû¨­^¿ëǵn6itAGNbll?îR}8;?£î¢šº±?¥–mS¶C?¢¹Ò‹Ÿ?…û³êâÐ?'"iÿ/?î+,ÃhúŒ?¡ÝRlÁx?¢1ðq
?–õÒÂã˜@?–6‡{þ¢=?•éÈnÏ?ìú1j¢òB?¢1èKoÜU?«Öì¨ Æ?šÀA,'"?¤…ü­Ë»?'¢ÁÅk/?ì EÏü•?¤Ðµ(F~?­/iª )­?–e
.ó4?¨Ðø`
?žíªfA3FGL J0802.0+1005@jw6â—@46'ßk5À:`2g[XìÀ;Ô:0}vM?ÓÈì²44@Œsk\š@*‡?Ïε?äø‡ç2¿×õ)¹Hß¿écí°r#3¿Öåæ<2AGNbll?ïrïí¡_l?'ÕçvÑd?‹v),ɌŸ?'W'©ò0?o7m«zb?sJ+¤,X?ïvû½i®Þ?—5Ò×üre?{½Þ,¤?ƒa>=OÐÎ?"³F¥2G?'Ì\#ê%†?í®qÇRŒá? ¦Ôœü&'?¥Ï>Ú¤Ý?™àãV»•x? Kü?ŒÛÝ䚼?í¨ù
m˗?¥À3	"?›Q…V~Ø$?šL3‡8|ö?§Ç¬­ãÚw?¡OnÃ<ôÓ3FGL J0803.3-0339@lƒ@'À‡@,[	 :2+À98'ódKÀ;kՙ$(Ô?ÓNЦ(ѹ@÷êï!¶?ÿðÁ¡J'ö¿à<ÐÀ¼¿á6‹ÐêO¿Úx¯IÑ}¿ã&oI¨¯PAGNbcu?ïìuŒ$ˆ¶?e|¿:
|??2ayØè#?+¼äêbï?a>Dº|+ƒ?dçœ[bÎ?ï0üœßù£?š´ZÛgé•?výóŽ,z?t8VLj?" @c?˜¹çœŸŽ?ïB]"Ñ?‰g¸¼(Ü?}ÈÜ"òó%?vË øµKc?Bvâ‰6?ƒ`mD7ÄZ?îu&èä¾?'ê4~ñ9"?hEôUÌ7?c-1  EÀ?§,-zgZ?'–+êz 3FGL J0804.0-3629@o¡œýç!À-ŸöUÀ9JⴕžÀ;êßÝJÉ?ôUi"í];@>Q%âg¿?ýAŽàØóL¿ãw»3®i?ïõÝà£÷Ê¿Í@X¤u¯s¿âŠ­)楳AGNbcu?èâoOŸÁ?Ä`L;½?¬8pR¼š?¨)go]Sª?ÆzZ.T?Ã{9~?Ô^'å×ä?ÑéõÂ4O¨?ϨցÖ.Í?È ÎÝë&?Û͈—/¶?Ð/{Qn;­?æYéouŸ?²1fIÞß?À¿h°Â³Ø?§u/P´Òù?ÅÜ©uª?­ó	Þj/?æ?Õqz¡7?Â*My[ˆ?Ìϙ?Á8ÜîOæ?µÿµB"ÐF?²!5ÁmFï3FGL J0804.4+0418@k/òÿÑÜ×@2/ Z8[À:9Íp`»,À;Î ž9%¿²ÿÖÈû¼6@bÎ
{@‡¾?Á6¿ám, 
樿ìSò²ÿ¿âu-yÆH¿ØŽV,\AGNbcu?ïôԅ´`v?X–è¾Ü?*

ãyc?.(Ñÿ¼ý+?S²ó¢÷?W&Ã^¢@?ï¹"—ˆ®?"¹ ã Ì»?h–%u¹Á?q¢½HÌ?w,³!€Ë;?}ì—.?ïü±žbÑ?‰U Ñ*9_?}I}Á§êÊ?vFO¤]F?•î
[ɪü?…nÞK;X?ïŠÛϓ`9?ƒiùQ‰e??°"§Æ÷?CMª³ƒòÄ?ŒK‡uï;1?'çëèY\!3FGL J0805.0-0622@lj	 'RT@*iݾŒ˜)À9Ð%E3æ·À;sŠ÷?g¿¹QQŜ6?@(©€—j?þQìa<°à¿î~»Þ?Š¤›£M¿â½Y4N¼&¿Ÿ+ÍÊ^ï‹AGNbcu?ïê2DWr?a!Lã?Fщ53qW?B´­ì‹?`Y[AÖ?]ºn"…Ê??ï^Îíææ?™(´oæ?hê9>/™~?rúàEPúH?'÷ú}0?–¶+tâh?îø½È"? ˜éµ}?†Klèùq?}tÃÝõ«?•Âyyˆ?ŠkìàæÿÜ?ï²5-Õ?z'Ä@È?:֞Ngý
?D8/J¶"8?'¤}­AJ{?y›•¤EB23FGL J0805.2-0112@kÖ3?Èlì@/—(_ššKÀ9"ÛVÓKÀ;¸Y_æÌ?àBñ¿þæ®@?ìsS4@·ô`d™³¿Ùv'D"E¿è4îV,¿áÄìÿUK¿è²+¸YgAGNfsrq?ïí‹Øieù?lªÙ1f¥"?>c³b2r?@Ò0og°Ç?]O‰À[€§?jñŒUì$2?ïÀ¹´ÁŸ?ŠœF«~×ð?iÁÜOhœ?kLÏM_Î?'Ž[»¾?‡)Q5"®?îìCъç©?Ž)IRyHµ?ˆõªDñ?€°9™
¼?•ü°¬*}c?†RJÛâ{?ï}·ÑC¨k?‡oÔÎÀ…z?X±kÔ>X?TÖ-|>DË?5›]ˆ?†¢‰¿¾aª3FGL J0805.4+7534@a\j~ùÛ#@>ʙ÷LÀ8Û+6¯ÆÀ;s}°/U¿ú'Cß}Ôl@;ôvH?þ®íÿ!ˆ¼¿ÙÁ‹EmóN¿ß©Æónø¿ÞMdâ­µ¿ÑkFÖºG AGNbll?ïý°y"šu?'ñ§™'Ðd?gxäTF¸?ÙFrTÙh?*ĪD."¹?$¸ôJø…?ïÒÿŽØeŽ?v«#;7ï?b`"(֕?eẗ́î'ì?j£qœ‰?q8'Èiç?ïlæžÉ?"GèIæ?|¡Á`vË?zÁ")Ê.0?†ÅlëÄ?y䛳àæ"?ïæ̸LJ?hŠIË>áz_@>ÀG>ù˜ËW³$?i!ÌÙ«8í?h{å	S?–3FGL J0805.4+6144@caA?ÐÐh@@.é€aº/À9öåvÀ;ãe§ú…m?ôIYÑÇÞ@_!CœŒé@üº€™îS¿ãã•Vœwx¿ëo¼™Ï¿ëÔ5™6j¿ïý2È1æAGNfsrq?ïð"‹‰X?hÒÍá)@?T˜|Eg´8?fMFWE¸"?D¼ÙOÐ9…?P±º•ÄF«?ïÁÍá1èñ?{ "–uؒ?mÿÍ®b?oØãÛOYG?p(Ø´?qTˆZn1?î*QDO0æ?™ÀS]õô?¤KÃé`R+?•Cf¾×?'O£Y>û?‹[ëPìŒ?﯀8®ˆ?†"U¼ÇÀ?l3üsD0?o'é+ãèk?z&såo?"Mz'#ù#3FGL J0806.6+5933@c³û_ïJ@@J˜?ýFÀ:c/Çmè;À;ïÅôkwGÀ`
+Òí@(õgJ¼è?þ€W([¿ïòÌÒÅÎñ?ïK™™C³^¿ëĎ*XKÏ?Ôb­WD=$AGNbll?ïÝŹñ®Î?vÅcÓ9NE?mþýM»?vQp÷ß/?DD
â?EIÁ6ˆ"z?ïÕ*Rdî;?wŸ…('ُ?`«fÈ	6Œ?f§¯åÀ-'?j*FÓŽÆ?qdá2#à?²o¶T?"óîómà?—Wvýž¿€?'J…¦"?'ØR´juê?ÆJ›Ž*?ïüpè…F6?M™¶'¶´>ô;$³9?ߕFýÊ?;5cƒ£?Mñ1Üö3FGL J0807.1-0541@l_?p]@,Ï¡"cÀ8Ât=¿~0À;BñTk'?ðM¥&À‰@2^?Pwè@‹°ÀQ¿:?ɒ˜Y¿àŠÚ‹É™´¿àÙ"v€›¿æB£•4ÉÐAGNbll?ïÊù'؉®?qð*ê?[û~OYP?cˆÈ•¦›?s"pt'R×?|ŠS\*#?îM·­™|K?¬Ué=Ä?‰l&T€²"?†•1:ÕÜØ?¤É{'H?©dÆì~Àé?íÈb•«ÐI? ¢õ[*å¢?›¸û'Ë?vNý`€Þ?¥Í'¯Ï?™ &$ýq?ìÄŒì?ªߙ15?›3«6¡?ƒà9ëU?¸4ôUð_©?©&ð'4®¶3FGL J0807.1+7744@a
¿p@>tþÀdß~À:*‡{‰äÀ<D™`¿é×s¾àóB@Ë,çêŠx@}/`jÎÖ¿è°—YoÕ¿åô©Ä\ß¿æµ´"xít¿â
¢ûd‡6AGNbcu?ïûä—}kL?I=ú($á}?4[œÑ?B\"Xæû?)‰Ðï©%z?5AäWËÝ?ïÍœc?yT՜æÏ?c¾Í·ÏC?f•9Ӛ?oËÁ•åü?s+ö¯ê¹5?ïÊè•ni?ƒD'_ÑÝý?}ܟ_ß?€\nì'â?€žöžµv?s:ŽéµüÂ?ïèü?dÄe&ø@¹?Ž‹J(©?!ÈÝ7»?gÇé­¯?dyŠÛ~Rû3FGL J0807.9+4946@e'ŒŸ¶M@@9»üÊÀ:$B_öàÀ;ò©1½n?ámyÜK@Q'H—sz@"@ªÀ3¿âœQ:7çÖ¿ãlº4ç	Ü¿ïÿô³à[¿Øùå!ŠòÀAGNfsrq?ïí€.¢§Â?g–þk˜¼<?Z5#ŠCÜ0?c^wšN??E"þ`Ù=÷?Tip–°.?ïŒþ֚…?[Úð	ž7?|ሢÄø?…8]•‡s'?}üø"?ƒ
Ö·?îö›½cM?a–;Ñ
¯?‹Dи¥?có‰ÜºÓ?"Š†g·Ž"?"yÉzÔè'?C‡'? ñ4®™Þ?•þµmn8?™ñßõ£fÐ?–?Õ
!y?–•‹°P_3FGL J0808.2-0751@l¡qÿ÷œ"@*Vì¡~jiÀ7/¬ÎÞÀ:¨Æ¨Æ]G?üˆ—'ÃÊ@«i«kG?þÕ¨%xŠ€¿Ý7I²~¿áå=î¿âuì¶wò¿æX|v{ºêAGNfsrq?ïÜDé™ùO?sMÐ:i?QF¢aÏ[Í?T;?kÅ5¬?q!£À-÷/?;eé,?•[¾î"6?]\2Rý˜,?f'¶XìÀ?…©êÜ&4?"8b¼:Ïë?ìJýHçÆ?¨Å­à^?¨€Ž¶{n(?›iCÿF²ü?³­`º{
Ã?¢Æ—aKäï?ïòÚpÔ±¬?g­ÃN:Ô>êĵ{ïH?‡ÁMÅæ?Z"ìy±~?gp™"ß3FGL J0809.5+4045@fzX`f@?ŠüAÿÀ:-Ÿw),IÀ;Ò½M#Ÿ¿ðÂ^18²#@Ô¾È}1Ú@3
ŸÐÀL¿åŸ"úÚbs¿éz§ä5E¿àF…8ʲý¿ïþ÷b³º"AGNfsrq?ïû:5ʄÄ?KP[[ó?L‹‰øûV?ÁÓÚ]Ä?@
—d­Ïz?IAârm?ïµ2Ðí?i?€ù@v;Û?púÈøS9 ?q*6PÃj?tkΑ
?vÁõÁTü9?ïhª* ?€ƒWn7|?€àÌAî?p³˜3é@€?…äØ	4_f?y"Aäï^Í?ï‹ô§p~#?"˜aŲÎr?J"Ò¨¦Š?R`ç\Ò
²?‹aSöµí?ƒ­$¤WE13FGL J0809.5+5342@d' 6m@@wÂ`b@gÀ9ì¿G©ýÀ;èÊõ\8?ÀµÿÅêÓ@ð›äøg°@A)Þ팿ßC߉¤X¿å÷Ù<5ª ¿èßÓr-nù¿Û¥Æ]ÇÜMAGNfsrq?ïù†±~0i?H+¤VSŠb?7V©bÐïì?>päèDŠ•?<sÊ««Èå?>ô×>¾˜p?ïƅekŠý?{€ã"ç`«?h«õqXý?jãÿfˆ?pgÁρÕ>?t,&܏ۚ?ïMê*ò§!?"MàšvE?'ë:ÝGëž?{Qj˜×
Ê?‰š:fKÌ?vsÈN[ã¨?n¢Ä»/?㉕hS?HLª·¢XÉ?MábÎÑ?~/F®Î?~®Î£†ò3FGL J0809.6+3456@gNà @À@>Y³¿µÀ: ¿ž(uÀ;›]np $?˜³âèdzJ@Ñ$—'?ú´WÀ±5˜¿Á½~r™?ï ú!Ô
àäíç
¿á©²;&ÉAGNbll?ïäå¡QƁ?p
À¼ß›?Nì/tàÝê?SÌ¿7Aå?c_RÑGà?jBäØ•?ï;yâ;?›t¥:ˆÙ?‹]v¸û?'#½PÌU¬?†4Dn€b?.é^ à?îäAm=ž.?áÀMÃ5?x¬ˆï?†á•|
?'ÿ%ϼ1]?†Ýª‹5Z ?îkCwFž?¤‹ú8_?žÿó¦m×z? þ-ƒ÷!?"—x©TË?"òœœLƧ3FGL J0809.8+5218@dÈ,ÿ§ël@@tw_²íþÀ7¦&áìÂÀ:É×5Ü[?ÀåRÓµ@¼ãÊ?SÓ?þ‡ ›+¿á"P$c?H¿Û@°ÛeÒÿ¿ÛÊ¢Ú¤Àƒ¿Ø	ŸÚÌAGNbll?ïûJ؂w`?DDeêY?[A«õ¼?ZWð±:??ÒkG›??BǶ^«?ïÕ紛Ä!?v¶dhèE8?_x®¬;õ?dÕ
>³¦å?j[ôä?psëv¬An?ï4'Ø`<?<i`½ö?x ­Hb!¬?zH__]?"ey¡ßô?Œ&GŸ.1?ïîËÚúÓ?b–SÜgú>ÒT¨d¼Ò>ã²ÁÜóÓ|?a*ú°úƒ,?b'%£›ü3FGL J0811.2-7529@rtÿ†]}À5n -1'À8H°?)áÀ;hþÇÜ¿¢Pä®qÁ.@t]%ÊêÊ?ÿ* Htä¿ßÌwgjX¿ß¿Ùwˆ«=¿Üб€7•¿ßæ.<îAGNbll?îK<›Þ¡Ž?©bȧ•?rCÀßË*É?{:çŽB+?©¾&Å?¨ ŠæÀž[?îWìýù¥X?²DvÁj?:åݑâ?œz]걉m?¢y­váŠ?ª!Fž80f?êÝùjò1?©såÅ6e'?¤Œœ=z¾?'[›–ñ?¾Ê)`ñ±?¥‡°È`º?ç9¬ý3‡ì?¶¨X'T?…8ã+Y¼?…ÍÜHÃ?Ðä">•Z?¶YíÇbY3FGL J0811.3+0146@k–gk*@2Ž³ÀŒLªÀ8NâWxŒÚÀ;6~	ñŠ?æaž39ñÇ@HUñ¤ª@D¿Æ©ó¿Þ‰ÚÈ/|¿ã¬Þâ貿àÚWí¢'¿åÿa"<AGNbll?ïôÂ%}Ç?QÔ÷Œ¼¯?)JE¼<}Š?oc_g?SRlLêM·?QTq4×ä?ïÄ'K)?(¹µò?cñ"7Z`?gE6k)þó?tqsÏȪ?}¤Úà³?ïTÒkÊÆ,?ÃÁ됅 ?y›3•â£T?lYŸ?ýËB]#=?|'Ôa(ç@?ï|§i2‡¯?ŠåÍ06?FSîÜ.S?K(~ ´ßc?vtpQh?‰ëü¾Í3FGL J0812.0+0237@k¢ ¼8*@3=`³žþÀ:þ?5ŸõÀ;'ÕÝÀ¢"^#Í@€èÏa҃?û"éž¿ž;¿äGzr.h¿ásà¸ù"¿Ôê~DdÅ
¿Ã—
f>AGNbll?ïúHCýa‹?RÑfʨ†?!åQåý?.^?ü¥x™?B¶¶lp?OHÀqGü?ï'%
ÿ8?¢Dט"R+?ZaÎm—€ñ?eÊtcÙ×?Œ*'ñ
A¸?¡àÐ%A¶ó?ïaæG‡?äí•¢?w¬¬qÔ	?p¤…+m.e?‹°'Ç^3×?}Kc©a
?ï÷'´êm/?W
øu=>aÄB‹h>y×\Ö]´?Pús¶?Wòý¾¯}3FGL J0812.9+5555@d> öð@@ºö€$}ŽÀ:3b-À<¦J'R¿²©É{TLB@Œ¥{úø@ã; 2¿â´®<œq¿ä'§n™e¿ââ~=%X¿× N+S=AGNbll?ïͲ6¼b?uŸä¡ã¾[?RÛ»³Æ€?T]•'¸?toö2ôÜß?s֊J€?p,?‹"•€n®?{¦úÂ?¼£‰´?{¯BöµÒ?~^DL
?îÁ<›'K?Žƒ·-4–?‰Ìôð½™?yҝ§ž?šñò%®ê?‡) èÞaÄ?ïKS"2Rà?‹¤¶ïîôì?h†×ÁL—?k/ñòå?""Í>½z6?‰¨D=ß3FGL J0813.3+6509@bÝß֔Í@@€0`À:Ž'‰ÚßµÀ;Ô¨·CΌ?ϛXŒÍ@
R¢Æ>_@'°?£Y¿ë	G¨'¿Ûw­ÕL¿á:,‡Ù¿èÀ—Ë@ä)AGNbcu?ï†ÎM¡é¼?Œö>J?€Öukˆª"?NçÓ¾?zëîWùÍ"?W¾¤W"Â?ï´'MËÑ?"öTPf‡?¡6?‡{2Ë`ÿØ?‹ºjPŸµ?Œ{c¶Î´™?î0ˆ`D,I?—QiƺäX?˜ë(‹ºò?Œ•ý©ŠÇM? åµà1?5è,nñ£?í本c«—?œÈÒ)ÒÎ?˜Í/¤ú?‹DñNñ?¥ŒN¡ó8†?–¬™‹n;3FGL J0814.1-1012@lütÿ†]}@*m{Ÿ³À8ú"mRÀ;L†ŽúÚ&?Åzm]À>c@K9Ž—@'8`Är¿åÚîÄÕmÁ¿ä˜¢dT¤ƒ¿Û+z	ää¿àDžt¨QAGNbll?ïÙæ1Ýl?£å½Ë9-ý?0*"lÀMÅ?Z<Xò"Ï?r
>Ê}î*?£z¤öƒ?ï;$ëŒô?›‡ÙÃíVö?pð0>¡â?n»…Kìæ?"™3ö~¸Ø?š
ZwÝd?î÷&@ä ?"ìòdã?ž¼RD%?xFç°¤%?™SP4Wlö?'Ïƒ2?îÆÉÿî½ï?'B¡ÔÛ%?M±^ð`÷Ï?OÖT¦¾tk?£š…R?'?¸Žò#3FGL J0814.5+2943@h£3v@>€'ÍÀ:y¼>§À;ëtZÏY?㪛u(@
O
–<?ÿ¦à©ùc¿îí(ށ¼>?èŽR€«a¿àÜbSS±z¿å÷/"ÃAGNbll?ï‰BÂý
µ?Š§±{~?~d±t5P?}-,
`?|ùí
C¦9?ƒ?ŠsÃ*M?ê•R¢‰?ÄnKÛc°½?Âß8hN<?Âùr=Û´?£™ÍjĞ"?¥¥"¥÷‰?îå:î
ߜ?­EØÉa?Šk•ÔJ?{ÞDö~ÿt?–"×TËõ?…×Ù®õU‰?戶ȭTÙ?¿V)+B?ѝÝ%i?¿mI†ŸÏa?•UèsV?"fEUy;3FGL J0814.7+6428@böW´@@›aßîèÀ8Žõs}¦À;}ЍK­}ÀٔPXÞ@ú­ê^ƒ@_û¿~…—¿â{fôîC¿æüN^v¿à¯±íè@¿ãNŀ'W³AGNbll?ïûÌ|çù?AMûYªª?†e©bt?Gìi&™?@ÔW3͍?@Œ…Ÿ‰yˆ?ïÒªWƒ7å?wêÖ#z´?aÅ^¨g†q?fï†ÑÄhœ?kIÔ`"œ?qÄ&À½?ïv	sï¿z?}‰CðÿVG?pMt£Hp?`לuìÊ?ŠVè²kér?zŸnVn–?ïñ¡Gº¶"?bÓY܃:®>Ï'>«Vð>çK_[]ÅL?\­Üë=-Ü?bËXÂWÖ63FGL J0816.4-1311@mYb¯È°@(AŸ˜À8cKB±ÂÀ:ßÄ"ïï?èÝÌ.A[ë@ß²ì¦ÜÎ?üméµí¸?hA¿µY‹¿áÔ'€]Ē¿ËyÓ
D¦¿ÛL'æ>ZPAGNbll?ïÕ<¹}6«?vs<Õ$?6ó°ÁÁ¦u?9Âãñçç€?sòh5HT?vq|>e¸?ï
™™ëè? æÀƒaí?t|»ýªZ§?v}ž¹tD?™¡
WìN?ŸTÙd K?í¿^Oéï»?¡ËºzÍU(?‹A&pi?ƒ~Ҋ
Þî?­)Øñh8? 
ÛðNó?쏜‡¦?¦Sl­?h1¬hy{?nèX"¯Xc?¾Qõ»g‹{?¥Ü.žãšz3FGL J0816.5+2049@iMfŸê%@;¦1_ô\^À:™8I©"À;ï"öW
?ÈJ]*lT@
ž‡½N)¯@?è`&0k?¸2Çä–Ô)¿Ûv<lí¿¿Ùì£{^‰è¿éf"6Þ'AGNbll?îÃìÆB$´?¤ºõ;1?œþè
H½?¡Œ!Œ%C?…¾Ÿ\A-?†whö·U­?îôŠ<"%	?˜bÌDñXë?"GêWþ¹?Š"'ì?ŒO9FÀ'?}'çýdÆ?í;¤4ë?¦Yö8*·?®&áÈ%hõ?¢B¹ZÒ? côŽ\i?b™Šî?îE…ö¿#?™êÊùqa7?"rI\û.u?†¡áÛTì/?¤b'òv?"Ó¦^¢s3FGL J0816.7-2421@nŠÀ€ù£@ïÝëÙÀ9HÏmýÀ;ohی¿­r†fSJ@Pkþ*é@thŸÑ—¿àf¾ ȳŸ¿ç¾o+ÜÒ©¿è^Ξw銿ÛîÂôdtAGNbcu?ïáÕÜô	U?iíüƘÄE?Gƒxçl»?HKZüášw?hcB-¼Ð?g]e5Ì,Ð?íØÕ?ÐÄ©?±¿a<¥µ|?nœç©p?qž±9§?°DnÄ.YÏ?±N®>r*ÿ?î<x"Ê-m?–Ú󺻻?GÕ[k?g2
ø?¤æ'odA?"BRó/?ïhDÅZzš?Š:÷Êù"r?AO· AÉ6?Eø·Åcl?'l问žk?Š2hÄ]ð3FGL J0816.7+5739@cû;@³Nw@@øÍ?¹SsÀ9¦Üx;{À;¡iÀŽ¿çð+‰y@mJ
jKÎ@ç@ó¿ãýæzÕé¿àǵ…Õ¹Ó¿ÙÖ͂»lä¿çj…QãøbAGNbll?ïó9,ô€??\¼ Ò·†"?8"ãÓáÐ?6!ÿàtá"?Sˆ
ˆ¤?Yl?uXb ?聾F©l´?‡¦y"Ü?u~ÝG¾àþ?|~î ?w¾cŠÅ€?{öAÈÔ=í?ïJè:f"?†µ¢/4Í$?zi±r
Ð?sǘáÓ_¾?ÞFË*?ƒ‰"êI?ïj#ƒ??‹ä÷ž­Õ–?Q7V01Ì?ZƒéËtâD?'žH:ôÚ?ŠH
k3FGL J0817.8-0935@lúš?Ffí@,¢9 4¾NÀ8ß¾®&˜À;G²3ÄR«?笃›‰ù@ŒO¥¯§x@YIàsÈ¥?§t¹f#Ý¿Þ7Áá
,¿á3צx,ë¿àï›þ< 3AGNbll?ïHbQõn?""'W‡œ?€o$ø~ªû?x»y´0?xUóù…?'7@Ó·±?í@| sÓ?·¢­žœí?šó九V?ŸÁ-]ìß=?®~K›ô$Ï?²Á<§:»Ç?í.4ëÆoú? õè`6U?¢Wôjm<?"Qª2½È?ªÅšO."1?—¦8D7Ë?èpfßNh?±S¤MAÄ?­=|ˆ•vÏ?¢ø5žQñ ?Æï`¢"«?°Ò&WB3FGL J0818.2+4223@fFˆ?Õ%@@³YLVÀ7a{E¼À:Ú;2Ûõ_?öÞÙ|ˆ'´@›:Ö@?ÿŠx»}š¿ß 0öܯˆ¿á~ñ`°+¿á"t˜¼¿¿æëÓ=)V;AGNbll?ïçê㴍t?]àSɃ;?P5îå|mì?KA'ê3§o?_ôI±hª$?We]m?ï"ޝnî?ŠËõõ0i0?{î(ùÄ?}ž•	Ñ:N?zsÞÏT?7¡Kkè?î»gsê^ì?–…pàïš?'rß4Ž!?¬i?— 2Nž">?Ï-¯èrÃ?íYÇ?§QCel?Ž0Mê{?pz'vQÊ?±mŠDuÊ?¥Æ{\¾x_3FGL J0818.8+2751@h_™÷L@>e;?q/À:30'8'À;ã:ÆG¿ÝS!@	«l'¥^Ÿ@´Þ?ä"¿ãÕgš1Þ¹¿èÓ÷4¬Û¿×ö´·Ø¿ïÿÙÍ|[AGNbll?ï"B¬ÞK1?''åm¤&´?qϔ>x÷n?†ØªIGJ?'Š©0¸?ˆÜ_ww?äÌ æ™Ìœ?ÐÀýSF"?Òa@t뗘?Í‹òåƒ?°ö÷ƒ<Ç?°ÅßՓFÉ?ì"Å๫?¤B¨ël§?¦,Œ,°Ó;?"wԕ8§/?°KŠãÞ°þ?žÌ™ "³?é8Ìt°ÈÙ?»/¢Ú:,?µ&ödêŶ?³'tOë¾?À‰RúÇyÁ?²Æ㥺ù!3FGL J0820.4+3640@g Á¿½ð'@@pÀOæÈÀ:³Ô®BžÀ;ã·N¶Fy¿ø~&¡l@Ž£?µ¢@Cà{Ö:¿Ü:®%•¿çk	¶©û¿âÑbk/#¿àIq	úÍAGNbll?ïÚ±n¬Û?xbÔZKX?Q¤#y}l?T0Z±,qˆ?l|ægp?uQôthaá?ï¾î鐩­?|p‹ÜRa?jbžÁ†ñË?m>ªŸÎÏ?sW;Öç¯õ?tï"è‹j»?î"C
·z?"æãHg?' r»	?‰$mþ5b?W+âÈ
Ó?‡ÌÉz¶PÖ?爫rHc?}Íoí¬ø?$l]ຠ?/ÅâG1Õ?…KñödW¬?}›—¡}À3FGL J0820.9-1258@mfbŸœèÙ@*SŒÿWc"À:w "@ºÀ;·+rt'¢¿òzí¿`¨Œ@€â¦Rå€@,Ó P—ó¿êâ=‹Ä¿ây'vg¿ÜõF""ð¦¿æh¾òæß?AGNbll?ﮑïÿ?‡¡"j†ø?`~X9H?`µ¯_¶T?€;î0î7ª?…Ì;¼þ•w?îÒ"'ÉD?¯ÊÛjoº?q…RiäF…?''øÖÔ¤I? ­36/6R?«æÑ¹»:?îK)y˜¥?–õÛS\}?S'6,ž´?ÿ}Ì|ñé?£#ŸK_^ã?'bìéd	?ï}ӏڦ?ƒ
¸¿~†¬?0X·‹¡'?3ñ"ÀëM?9Ö$ç?'Íï}X~3FGL J0822.6-4250e@pE•:À
5ðŸºÅäÀ7A9†3‹À:H{$cŒ—?ñÏoÏpÁ@}3¤GG'@iº?V'¿ÉŽ;l'¥¿ã3݆Xt¿ßŠRiY_î¿âýŠoZ*ïOTHERSNR?ÄDgh7\?¾JAãC,?¾|ÂÙ|Ž@?»¢ôó5¼½?çMݶ`a?ÅÑáyLïï?Ϗ>`~âd?̟òy¤Ÿ'?ѧ€Òѕ±?Æ£ŸÔÏ´y?ސßüîù?ÉvǤÇAö?Ɠ/¡¿t:?°hñýÜ?½'(âÓK?§,0òÌÚ?æ¨îû5Á?´ºªJKŽ7?Ã833¼ô?®NÄÖB?¸mÉ'?­šÃha>?èA19í?´7™( åÚ3FGL J0822.9+4041@fŒ8¾øγ@A`	UÀ9Ê";ÝÀ;¯ÌÐþŠµ¿ß®Õ'[°ø@©F>RÌ@éà‰¿ä—ìëÑì¿å¾Ó¨'·¬¿êîCe'¿ÑÌÎû%OÆAGNfsrq?ïøU§¾­?Q嫶Û=?4^nE"?a?2ŒŽ#Ù?Dz)äÓ,c?LŠ0Â]¬Ä?ïÊMÉ"•?zKxC
?dhÈÿiÜ?h1‰Ì'p?p'g¶?sšf%ÛU?ï{Ž:[?|"u¢Ø_?ušŸ›JÓÞ?j°ol˜b?†O!›•Z?vö³—mÓ?ïкª×Ö?tÖ×{G]?&ÛÝ>'Ø?1Í÷lù½Æ?w=Éóª ö?t}¢#*ã3FGL J0824.1+2434@hàéߗª¬@>Šô PmÀ9Í]®1À;¬'Ä"Bh¿®U;¾˜Û@I¯K‡"@$e –"—¿änǬZ/¿ç	®éî¿å—÷9v²ÿ¿å°¾Õ˜AGNfsrq?ïæµSÆLû?j†îî#‡.?E	¡–@?Dû–xû?dCòn_C?hÇ¢B"˜?ﶌ%a–?|w|ˆ),?p@óÓËõ?lí®—ûÆÇ?txù¡¶h¢?u'£p{d?ïk€¥´‡û?'b•…u‰8?süM^`sæ?fcòϹÐ;?‹!¯ã­Ç|?|>¹¸g?ï9ñŠ®ª?‰ˆ¹>æÃL?e^PÚ•É?]à_b™Å?–Žï·ÿ?ˆ¾¯Á|ëó3FGL J0824.9+5551@d?n «†@A'Ÿ¸—ŒÀ98cϳ1À;ÑF2ê8?Á ¸è®@¢é¹íw@ÙÃߓMû¿ã\<´š¿ê^+œ;¿ä²67ìÍÁ¿é—ÐAGNfsrq?ïú¹¡B?E÷ÛÐU[u?"òxˆ?$â AÖúÐ?@'~W©ë8?C3i/
¦ç?ïÌǼĜ?z%ÔpÆÍæ?e§ñ¿)|?j°4û)?m'BŽ|:­?r¤§DC?ï@E˜è›ó?†ý"Výb?x‡àÿg·?l
þ€f‰f?'ÕTÞì§_?…+5«9
Ó?ïåŠÃ2ê?m+É×u¢D?&tà©û\K?*ÍE—Þù?i¢2-`Ì?l¿¹èlp}3FGL J0824.9+3916@fį_Ô{î@AU_­åÀ9Ć4b\À;Õ½5?âm¸¼Êv@jŠ'T@>`
ø¿èžŠçq‹¿ÝZ"e'¿è(ð@¼«¿ïÿà­Õ:ÚAGNfsrq?ï²=þ!ö'?…rmè64ò?'N¡
to?"ìÿü"SÙ?BÝgP!ÿ?Fm4-àÔÿ?îУÉ%?§H×´Yœ?£ù"´~)?¢o?Àìî?•râ6jÂç?•¢\tå;?ìr?¦0ç7ãùÑ?¶è§îÙðÓ?¤Ÿ^Î	ý?–
?C†[z?‰¼š¦+¶?ìi:'‡~(?¬èI	N?µVÐhì4?©Í>â$a?žRmlŠ+?•á͋'œÐ3FGL J0825.4-0213@lFÔà—"ì@3®Û@-¹À:S¤A"HGÀ;Ïçû&|l¿¸Åb$Lm@	2Á濽@5œŸ]}ß¿ç\ÄfZ6¿ä7;‰ªˆ¿æpÇNaÖ¿æƉ"ßgÑAGNbcu?ï¸TŒ¯?"­½—
1­?býý‰¹—þ?e7KÓ—
?zVñ«ÜÜ{?ƒw0>Ï&C?ì.Cgc?ÂKLÂÀî?²"<´J¤è?¶Rú
«‰c?©¶¤ã4@?µÄO‰}?î_‡"(?"ùÀðÐk
?"&PÊp†?…
QÕA{?¤ß"µšŒ?!)	?Îù?çñ'u1N?¶%i˜˜?ºoÊÙ1=?¯æ5·³.æ?Ãáõ'œ9?°§«š–Œ3FGL J0825.8-3217@o"Àh¡@
i¿ÿ´ÖŒÀ9d8Ž¼ÇÀ;Z|¼A%¿ýÿÈØK†@{ âù‰ï@ê®YÒY¿çq¼*	¶/¿äó®é¿ä§Úb{d¿êk…xêAGNbcu?ïæ"47HÃ?g[ø•¿0?Kd¤"€Ë?Lhž'?b¢¢§†û?cš´l-?êîµCøQ9?Ñe	ÔÒç?qŸ÷-ìrî?"¶o<·&w?ø+6¯Wˆ?Ñ4	ßU-??í­¯Qq})?›ŒVŠÎ"F?ž¯*à1$?'"©M?¦#³Sxç?"½'[ãP?ïôüýi?\}KÑc]E>Ê*¯ìz%Ú>Û2¢Ù•ä†?Wºð­ðð?\wÚoˆÆà3FGL J0825.9-2230@n~à°¯`@!Ùäúœ>À7ŸA¥ÃtÀ:Èï'j¨?çÏ™à@4%죬Ã@cÀCÒh¿Û‡y§Çëοâè$Zìú¿ÞíñN{'¿Ý>"[U!AGNbll?ï¼ÒAR¤÷?Mp§æØ?Bø
cl?F‹=ª>\?7ݪ@'?~Fðçý¤?î^´ª{?®HÎ;'í?wƒsâÚU<?|ã¡j™Ø?§/68ýÞ?¬­û@ñ/?ìùU3èÈ?¨!¹bsL?ŽÐQÛûÇ\?…LqÂË3u?´[LÒá@Ø?¥Ôé%ki×?ìš(ë›Î[?¦€øZËì?k-B…ô€b?nƍp)ʁ?ºUNŽñé2?¦w'}¨|13FGL J0826.0+0307@k¨ø -à@6mÀÊ`À9Ýa…V¶À;¬½D¦"¿ìïAïíö@ 2)gW@<Çÿ]˜·¿äàÿÆì…q¿áT'8§;n¿×ô'ª,¿ã)ç/#¯AGNbll?ïúO§–ÛË?Eq߸'/{?sdîM47?>•9äW?CRõÇ*Í?Dz¹ބ?ïÇS6)M?~ª:)g?d68œí	¢?gEäàçO>?r;UtÔ¢?xڈ¼¾?ï¢Z€­7Ø?u` ñW¾'?lý»ÞF1ì?bȵ+ÍÓ?€)ðÝ }c?pǕT½?ïµÔbÛÕ?tU-{ål?$4ŸTJ?"°Cu?'NžßÌp?t-Ô½·3FGL J0827.2-0711@lޛ6†¥@1Š	cr–À9ë:^ ŸGÀ;²ÔG'‡¿	äÐçž@
j°ëoÐ@‰žŸgäÁ¿ÞÔl´Z¿è~{å˜d¿ÎƒÉÈò‰¿ÙD÷}$™AGNbcu?î˜?§âï~?±)
°%ë?S!$ÕÉ?PLJË'8Æ?¥âü["¿Œ?±#HÎVz?ï€Ò†‰ä{?'Xù©ÆÐM?s)…)>?wªNØæG?†@PÈÄM?‹Óý"wÍ?îHUŠ
?"L¹V?Šbý,ËìÑ?yÀx¹Ç?¡Uœ/td(?g
Ý{ŽÍ?îÃggzI?'ª¾"c?S¡‹/i?\֕G»?£1,|¾<?'x.3Æ%<3FGL J0828.5+5217@dʽQï·@Aã(CìÀ:ÊÐþŠ´úÀ<!‰X¿ºáӞf÷ @g¤Ôá@'¿ãZX¿ëê)1°.å¿Ö6¯¿ÔOÙìðڿ당Šá×AGNfsrq?íi·ÃČA?ºæV±'$?´7Œ´"´?ºÊê@æ ?^­KUºwj?d8z5ˆ…?í*-™óm??µ"nÁQA?®烻?°}›)sj+?ž~4òŠâ?  °¯n‰?ê]ôÈB×°?³»13ò?À¡ô¸ãƒ)?²Ô>p(ã^?§˜à˜Dx]?—B8=vˆ?î[÷X±?œþÖòŽ±Ò?—ëÜãL?"ó¢ä£÷?Œ•8˜™?'åkz'^3FGL J0828.8-2420@n¼WÀ±5˜@ Õ¶`#× À:6ÄíÛ:NÀ;±Ø{V¸¿æP˜#Lá/@
Ū‰€ò¯?ÿþ½?'‡¿ÒLS'ÿ¿é×:$ȿȏcüï2¿ãˆŒ£^aAGNbcu?ïLÛø¯(?£±k=õ?;Ø&Â|‡??rÛ,òA?•õ;eà(ò?£ŽG€lŸ«?íhfý€Ó?¹6֊ó»?vf$£?|ڌšYΏ?³V_#·?¸få-Z;?î£ýf7¼?™
À}n‡?ŒY""i*"?|Lž¸ó1?§w¡9«?– ×¹Ÿ•Ý?ï3ãYˆ?Š‰[§í˜?-ª-m®¼?6ß	p a?™b@óÅ?Šg—t®žà3FGL J0829.3+0901@jý؈v\@9ÓÉ¿Ò‡À:¨L…ЗÀ;à\KZqf?Þv~;U}@c‡'ÛåD?ÿ(ÜP'`¿ïÿÕYu?ïýv8t^¿àò±C÷.¿Ô÷P0;~~AGNfsrq?ïN'O?Yƒ¶.]'?Rê…P¾_?R*×0õaÏ?KØT%æu?LÐVR˜ñ?ÓÃÌ?©•JÑ6~Ë?œá;…¡ƒM?¢KšÞ)Œ?'nJf:?–Ãt{÷`?ï (Ñp…?…T×W…è?†-î­h'?y(í}{Ò?ùe{;!?zè
<$?ëVȶ¼.?¸'
_ࡳ?¿Óåy§t?·žeÿO?•îŠªU?˜–Wcl3FGL J0829.6-1137@mf[ ¥&–@/\7 þ}IÀ:SÐ-hïÀ;¿ŸàÛwŠ¿õb ¼8*@AåÀ8À?þ;Úß_ ¢¿Ê±¡NU	¿ìF»,Þ§¸?Ñ~°ŸšŽ¿Ôr¨©ïAGNbcu?ïôØÎTmÇ?x®ù–H"ú?F¦•,°?ÅPiýß?UT2'ïÄé?x—@"é×?ï}¯[Æþ?˜høWŕ¢?bk£Á7ô'?g…›«??‹ù@,@CZ?—Tj®n6?ï=ÂNSœ?‰'ü?Ã?|Ð0,?t¯Åø:À¨?'VnÁ€ƒ?"jæO0‡˜?ïæþu°°2?g]¡¦bd>·ÊËAòª8>Ñ<á‹kß~?hþõçŽ,?g\€›°«M3FGL J0830.3-5855@q%ˆ¿Â"OÀ&ã
F:À9Z¾ÝöÀ¼À;†aQS°?è3ˆ2˜ü@=òFƒòé@Ý»à~í¿è˜p&Œ9¿è¬-ÎFl¿äÌ~?Ã\¿ïÿ¯í1àçAGNbcu?ïÌUA®#?€µ§Ãè¢Å?aù¯¼Q§?gO¬44­?p؝º?y'®^•Éµ?ꭔ^PÚN?ÀN60¨¹i?¬lø£­šm?§µ«.2?¼\໢`Y?¸}4ÍxfZ?îvN×(I?•AíÇRö?™JyIowÉ?Š'!oÒu?—ë«Ñ?‰Xé{å
²?êÍHt/æ?«vÛ
ž?¨?¯¨ÙƇy‹?œM³Jÿ?¿m(ÙÄ?©ŒºOú°3FGL J0830.7+2408@iòà\̊@?Ô· "À8¯â*ðoÀ;'çf¬"?î,Û`–÷1@è]…TÖ@í?³õ¿å@É-}^¿é6ÀNí¿çr
²©`¿ìm«ÞöAGNFSRQ?ïñŸ8óÒP?Sù'®®©?P7:x¤…ß?L¾tzÇ?I§?m±º?E
"§¨?ïz"ªG¹ü?Šªñºº›S?'‡B—à ?€¾…Â5ä?~¬œVó{k?€ˆk{(?ïÂì7ãz?îüÓ®6ˆ?TLÆý	?ƒ¥'àKŽj?Žæ«d
o?'hñ»þ¼J?î6žmË»Q?¡ÜYeÀo¤?"a_K¼Eq?"MÖ!?¢ei}f(=?ŸFAMæp3FGL J0831.9+0430@k–Š r~@8^'ŸªTÓÀ8&–5À;9¯4^¬?ö wÔÍÍ(@*íEé]@°Ì`Á5ë¿Ú~Oû"´õ¿å
‡òÓ¿ä2z ë¿çC^ˬ*/AGNbll?ï󠱘Æ?TšÙvžÎÊ?C Ýïµ=?Iݾz˜Ÿ?N^çI稏?Id Y9!?ïɋ5V'à?}¾þ_õ?d…:³B‰?iº	bÎ¥?p÷Çû'o?vø܏C?îóMôQ2…?'ßdÞa©?‹Ë›žÍæ?†5…°ÁoG?"°së
H{?‰¶HF8?ﺶèRÖ"?ƒ
*ŵ3?GÈJÞ]Ö?^¸0	—Ùn?¬Í9#4?'m~‹Y3FGL J0832.6+4914@eC[ÿW~@B6| À:¥kÏ[óFÀ<>ô1•¤¿ÑHe²¿ãä@
'žÜsß@è? ©Ù-¿ºä¸·þÝ¿é+'Ÿëñ¿àöäð§j¿çJ+í;#ºAGNbll?ïf¤¦ùl?"Tn›Ñå?yPf
*Û?ƒ'l["?‰®¬'6i?7ÑP"?ï† ³ô'?ŽX <ìÅ?%Gì67?·w…8¨?}Ê^ä6h?'¥µú"?íÌN¶‹#ƒ?™Gq›Œ¬?š‰þ/ÁŽ?³'',Ý	?¥öm??'­
Yã•}?ï¸y¼ÿ?'ŠÖ:•Ó~?o7nÈ*´?f <Ö§i?˜"¦˜?dàúa—º3FGL J0834.1+4223@fSëßL+R@B'±ÀoÀ9f:¢"=_À;Ȍ{£åM¿ôž6ìü=@<¦Ú'Q@ƒÀ`óJ¿å«cÛi8¿ç©Á‰Å©¿ÝTPф~¿é£Ü^nAGNfsrq?ï9̳Þ"€?¤~!Åá²?zãÍhÕ?‰úåÿMÀ ?'
v*mî? –'$;B?ïèˆ‹q?‹
ao}†Î?yÙZåʽ?zb!ð?2õ`Ô|Ý?ƒ—Ä‹C!s?îwMî9 _?—
9y;¦?w>ŠxµJ?…õ˜ý
? ­QyÏ̵?'/•.–Í?ïdQkü«?ŽÖ±æcœ?P.ãóÔº?`Ç-þ_?'räN{Pµ?§³vM.Ä3FGL J0834.7+4403@f^Ñ·@BH{Àj¾»À:l{¯£ÇÀ<Ä3¡<À¨ˆ‹ªB´@%š_'6Ï@½:¿™ˆ}¿ê#"±*ãa¿Ïh
Ô"	H¿ä&\tŽáô¿â7ÁGˆÁAGNbll?ïïبtªR?"ù–7õß?]JtwB¡T?"ú+·
Á?(!ÔûEËf?#åÄ4¦@?ïҍsgF?wÏ [7þ[?bßÉa‹?gqì?j'Ãù7.Ç?q¦´mžï}?ï-¥ð¸¯?‰ù±nW¢?‹Uë3jð?"{öòEJ?‰Ž.Þhì?yª)pó?ïôÃÊ^T?XmœIKØ»>ôy՞'0?®ÓÜås?V&ƒí{#-?XS#l²3FGL J0835.3-4510@pxß¿ƒ8.ÀLV ž9À2ˆ©ÀXJDÀ8Çå"S·@衦ˆ›@ø9'rÞÅ?ôž£¼ˆ1¿Ð†bbÔ>¿àÝskâ¿å>¢ÔšS¿ì̋Ç0PSRPSR?.YáþSá?IèA(~'?å!#¡0â?ÕÑÜÍ·t?ÔÛò|}Ýò?ÕÐfŸÔ?+Ò»è+ì?`¶Ì+Ê?ëЖ¡˜?ÉàßMZÕ?À¸´ö¦?Éâʄ¹‰E?jý˜vWÏ©?tÉh¸8P?é4±²ì±"?²+gËÃ0'?ÊÁBÒsÚu?²ƒ>'o>]Ñt¶Z">~…iå³¥î?ïºß½Y?•,‡ù‰¹T?H5j&)?•,…ùí2Ö3FGL J0835.4+0930@ko?Rü&@;fi¿·:"À:WozânÀ;Ô$n:¿Â"+l=@³ieIZè@OÉ Gˆ«¿ä'Õ""¿êV_T?·¿Ñ©Îée<x¿ßoò2bAGNbll?ïÁ
ϛc7?Oý°`«]?Râb'‡ˆ'?Yý"uG?zÁÿì'?õÞйEö?ïhfÂqŠp?rÒnÜqÍ?Œ#M+g?'u¬R4U?"Z1@P8M?†	Œ
Ðc?5¢Ú÷?'ù±S'ë?Š'>J—?~om£U?¡AÖJ}ï?ŽÉ4XmC?îÎ|ÒÈ?–UY݅¼¿?e
",ö?ltãŸNÃ7?¦'nôð?•©‡>zR3FGL J0836.3+2143@ih*Á	J,@@$ÓÀíÀ:K/ÉgeÀ;Ô¶JªH¿¥ŸtD¸{8@
†Ã(3P@†š@ˆ†L¿çZþÞdFH¿èð­&¿2¿çÙÔ5ˆ^¿Ó(^öQø¾AGNbcu?ïû˜DZ?BüüˆLC?2L&ña¾Y?4ˆA´ûý?5¯ø`·Ö?7(­Ø¢Ïä?ïȉ­èÍ?}|ÿ×ÃÔ ?f£ôwÛ ?jžzi²éÜ?pi}í
1?uë
›f›?ï'
ä3î?z¢\C}ýä?ré†Åèè?p5w…ó¾#?'ü/ÛY?rÒóþh"?ïďËP¼Ž?x-8…«5+?7ƒ&Ô}ì?>Û¬¦Êø÷?|?çötq<?wԗ®õžr3FGL J0836.5-2020@nsŸ‡ð$@([qàíìÀ9"ØC""À;¢Þ"umj?Ø[·Êßõ@ - ®@Û$¼"Û¿ècpÎQ宿鞡S!e*¿é ,W™;r¿ïýÁ\‰ÌPAGNfsrq?ï›Ï¤Üp5?‰wb¢©.¦?qôçnKZ?sð·o°?€£H,Íl?ƒHz/5ú?èmš¯©©>?ÃãhÕùÜ?·°þé|$?±d'Ôª\?Âq"Áäœõ?À"&(?í|Øøº
M?œÊЪ`Ù?£§WZ¯Ï¾?óy¬@'?¤‹¯[n?'"4ø«Š?èA±Œý?±dy…©a?À"3B?©S@#[k°?¾Ç]æw–?ª€îÂYÙ3FGL J0838.1-4615@p‹ƒÀ~à±À\ `ˆ+À8$›†ãàÀ9¼n9™~Â?öű:5¥@ï†<š?ÿϾúQ?c¿Ù:E E›¿ã3õƒ¥¿éµŒ©ÇG¿î¥x?V×þOTHERspp?£a$'&µÔ?§ºx7Ð?ÈB?´zã?È%ߨ¼H?è¹]ñðuë?Ê©
Y=ær?à¡.g¯uÃ?ÒLn±ºÀ?½ëAƒÊ×?¾lšãI-?×z¨`@!Ä?Îàüt""?ĺ+Gª?°>zPÿv÷?Ò²æh±¨M?²3ýãAė?áx
Uj/?·ž~T?À'¸y;P?¼SÙt"Ïa?²ãܔê´?¯ç=Çg?é'î@Ö?ÀÑ~e§Ž&3FGL J0839.1-4739@pžæ?šIÃÀ#Á`]öÀ9¢t3®ƒÀ:ZQU]*?ñò÷c#f@âeæ9@®èŸf7B¿ÞŒ£çÑ5¿í°˜ƒïä)¿ìZ¾b¦¾?Ç¥}=OTHERspp?ÇÄ4×}ŒE?ÅñîŠÜ…û?Ä_ŸY£¶(?Ä¢4ûˆ´U?ä÷
ó·¯e?Ï­67¿Ã?êgto²Wä?ÊB
ë–?™gŠè 50?ªàï-µ¶?Ã5<ä"™Ç?Æ¢S9&~å?Ñ0å|äd?±@–¶d\ ?Ìí§Íƒz?²ëéWÿe?à,#N,ïs?µÈSÙî?ç`Äé"i.?Ç¥rNT¤ ?ƒT¦pÿ"À?™ð="ùÊ?УÐùQ4?dž'Úu­É3FGL J0839.5+0102@l!O?Ù3ã@8_L?s³VÀ9È[[piÀ;ďñz+??ò%ëú}·@<'è§HÚ@æ­àMˆ¿ºsçûž¾¿¿à‡Q¿ ¢ô¿äE|	w[¿ïÿ‹Z,$AGNfsrq?ïDP=h.ì?™8˜NG"?•öî}ß?˜¢þº°_?Wð¤'Ðk-?^½•^þKp?Þm'L?Œì¾ê«]?}ûë¿f‹N?€wu{âë?€S'"èg…?ƒ0°åûB?åÇþêîXp?²ÏÕ ä£ò?ΜºGFFj?°Ò+¼Íü??´†"¯¯? ìÑn¨Î?ï$I?ÁL?"á|(×v?‰º)•á[?†­K÷QÃ^?3'¬yËs?ŒsàŸJð<3FGL J0839.6+3538@gcôŸM¡@B>n¿Ñ;ÇÀ:w»"€^À;¾–ä•?ˁâmÈÛ@
íæšÔ,=?þÄl@šúÿÛijãà¿Ø)ÉMˆÁ¿Û§7á\•œ¿ã°UþdIAGNbll?ï"ò@³î‡?´o.'ãÚ?hmüqtÖ?jjŒhì?"§ð¶§(®?|(»-‰]?ï:¨ñÉÞq?'ûìeRÇo?Šæ=a@AÇ?…õ"F~ý?†o†,H!Ï?‡"}*¶Ìž?î×Ój'?gK¶'?cHæQ!°?'ÞVT{ ?–SîL¥/#?ƒ'ú¦3§è?î(°É$~_?–"Ñðf3?GKNàì?¡¶L>´L?¦# šÂ?"J"ç9^r3FGL J0839.6+1803@ióÿ`Ï‰@?ÁúàŽµÀ:g8Yã¡%À;Û²ìPö"¿ñ~n¸Œ@WÕé4-?þwæ Zé[?µ&Pƒ{H¿ß3pÍ?ð¿Ûÿ)w-ð¿±bÓkÄÁˆAGNbll?ïø¡åÑKÏ?Kƒžzi]?=yˆ\ý={?A†'0p?=wI¤Cˆ?@+ôÃr9?ïÑMã-?yy駆	?c÷æ2æ?j.0éñ!«?kãìËéî³?q¯žÛ?ï#1æÊc?‡[IáÐêž?‡'{P"ºu?~¶#0Ò?¡
üëlò?z§œq.qÀ?ïÜy?Ù»µ?n[Aõ¸Y?2ãi5™¡?'­¶Ïµx?q úLOºJ?nI&
	‹E3FGL J0840.8+1315@j›Ÿ˜·@>+?8$4À9¢Àøƒ3ýÀ;À
éh?ëz¿Ôäì@9Ua0r@¾Í­ð>¿â5JBï>¿èy$ÞÔÿⴛ<Ú«¿ïÿ¸ÕҍŠAGNssrq?ïøpœ‡Ð?IhþÀD`?+kÈ|éØ?%¤q³Ño?Gu²ñ­"ù?GŠV{-ý'?ïiók'f?Œcž´‡y?ƒm¦>'–¹?€ÒËöçëv?'~üHÏ}?'Z^Ƨ·?îø'³Ÿ¿"?ŽrÕéLt?jÐ#sߌ?ƒæAÖ9h?'Ùh"<B?ó¹ò7-?îãr]M?• Êm³mQ?Šøž¢_l?"g‰3Óp›?–Š8/Ù?'ö6Ì‹3FGL J0841.3-3554@p
Ձ¥‡@
æ1ÀAyÀ8 TS>kvÀ:ðÓu]z/?òã(­"÷@tpȕ?ü:¿ë½Ô¿×¿¿¸èz¿Ö'´ƒ]v¿Ê`P¶6¿ÜòàèbªoAGNbcu?îç;KOšà?¡€`äÆZÍ?fÎüòdT?sãaRš? *N[7+»? ÑŒTº1±?çϯëþìŸ?ÏÓ´zP?%!=%'@?•´M‹OJ?μœ(_›8?ξ	.õ›h?éì°|]¹ª?°b똷?¥ý#"Ø•?"‡òÝ'O?ÂÍõ-Rô?¬‰ã÷ñß?ëóJ67e?«Äa Ä›5?~žTíZ²­?ƒ¹û4®?¾{É€™®?«[-·Ô3FGL J0841.4+7053@añ'à@A7E AYÀ8	³;+O9À;€æàtI~?ûÈ=ägF@i•šÜe@<ѯµÄ¿æ›BŒÓŸ¿ëŸÏW…g¿ëƏ¨Ì^à¿ëÆl:]@oAGNFSRQ?ïð'ª9ò±?[°¡JC†_?YƒL¹Å"Ë?Z4ï6?5e{IT&ß?5;.Le»¹?ïÒZò㵜?y•óY9é?a°œ?à?d÷Ÿ¡jã¢?kôpÜjRÏ?tW)Kœ—?ìÙK—u÷?¥ÀpŸv^€?´SÍ©{›?£ÖÃÏàaf?"‡Y
«R¯?·Ä³¯çX?ïõCħF?gb-@T¼g?%U€×S…€?LŸ£/g•h?RÍÇÅÇZ?fiE}y÷3FGL J0842.0-6055@qN9¿ß~€À&Ð[À6ãÀ9	füŽ[xÀ;z³Z4ÿ¼?ñ0èóžó¡@¾Ù>Js@ŸÑÀ§zƒ¿ã'»¢Fֿ嵊ÂÕìË¿àé4ü®^D¿í#ÞùÂqAGNbcu?ìá'>OÉÖ?·À¸'K?¡Pž<'–? w01Ÿ²Ã?°Kžÿcgþ?³SÂ'P»?çªä}-)ï?Ç/5È^.?³ƒ]†Òga?°s+ôz^?ǒ¿Gâ$'?ÁÄjžÆ¼Ÿ?묯ÙvÄÄ?¨sc—­?³}û=pm? DZy‰–×?®9ZÒæ?œ8$çX¸?ëRf6K?¬2 lFÃf?©áJ–¡HÈ?Ÿ­…,Ïìk?ºlʁ}©E?¨Ñ0ŠË‹3FGL J0843.1-4546@pÏ`Z³«À{=ŸrÌ{À8¶Ôš÷g«À9ïg ù	l¿òŸXj¥:b@Í­ð>@D5¿æ+Å`qÚ¹¿é8"ѳ¼[¿ét5A*l»¿ÝrFnyZOTHERspp?ÁªŸÄºµú?¼â&7"."?¾´ÒÕ~À?ÁÌ!'/Ns?ç¾½´0©?ÈƬ˱"à?ëæUˆ¾÷(?È1‹Š<ź?…"«\øß?'DÇÝu¦?¾𤜧°?Ç9ß 8"?ÐgfÖú?±{EŠ¾ª¤?ΑAt"
?·>ø?ü?à((o'z{?º8ycŽl­?äRýç{?ÉÁBZí½¥?'8kVë¹?2äùó?×W0‰žú?ÉÀ>G1ãE3FGL J0843.9+5311@d¢KZS3@CÒ_³Ä¾À:è>BZîÀ<‡ªƒÍ?¥sÀìa@UÍÕ
ˆð@ëõƒ¥¿æM¤_è•M¿ã‡:]N*¿Ú åÓ¾
¿ïÿ<!H"AGNbll?îÒQš["Î?£õ»\où?˜düׇ¦ ?¡Ñ\XñN?Š¡Ÿº¿œ?Šn)Tdö|?é­°š"Ç?ÂÆ8l®+?Ã{E#!ùs?ÀDœ‰†"?§7ê©ÎÍ·?¦ài³œˆ?ë©n,ÁÏÎ?ª¶Us—‹†?µì'9,t?¥çi¯Ñš?©Á¨ªI?—G¥,a[†?ìôš¾úCÎ?ªì¦¸DQ?©êuê`v?¤ô'ƒz'Y?¦ËÞ%û«¹?œ{ouÀ3FGL J0845.1-5458@qT@(äüÀéá€8ªÀ8µ|N/8À;G^X?éˆu¥@X8ü÷@[=ŸrÌ{¿ávý¨À[®¿å»ÒÿŒ¿á€o$Ç8¿éñd—ëTÞAGNbcu?ÔR˜ú	¼?Ãþzý ög?Âßå–>hk?¼ò&V,²?áGÝMóa?Ç˨áV?½q†AÈ?½*oÁl?Þera¢"?ÇÐàrÊU•?ÚW±<Øíû?ÅÂS'jÆL?å}™'ÿ¾?±æ¼»e4?À³àm7Ò?¦>ú{əÞ?ÉU»p¼î6?ª‰-,YËt?ցÉŒS?·ƒVWø"á?ÑÞüN¸T?¹rû(À'ñ?ןîè2œ?¸k8? ¯03FGL J0846.7-0651@m,xßzN{@5Φ ™@À:©-‹S†À;Ãý…Ò<x¿‹GÿFô+@	 ¼c1@Ò[ßú¦û¿ävÿ¨r¿çêIf~u¿ç"Öì‹Y¿ïûõ-Wë¾AGNbll?ïŸZæ/(?'ÅX'°?eˆ¦4R?fÑy°…¦?'¶\ç!¯?ŽÉul-"?¡¿?§9G
´q?¡p;ùÆýÕ?˜ÌÁv©"?™Í—8NÌ~? ˜[hø!?îA•ß"=?•Pɀ´'?˜ã'uÜk»?ƒ«¢Ü×?žéËn?L?×°T_\'?뼏t‹4³?¨zlª(]?¬ÃIi›Ù? ,.‹k݌?³¹ß¦Ø"r?¢,°yE¢3FGL J0846.9-2336@nøeÿ£¹®@(i'¿°"˜À9	åQþÐUÀ;VZU¶ëº¿ä@$ýTBç@¯ôüåš@6ãtt¿â@")N>¿àö¸dq)õ¿ãÅ1˜±ð±¿·eÖÞôl¤AGNbll?ïϝI+ÞÂ?vÁ7'ØÝ­?EÊ,™¨4?Bݛ@¡J–?uxÖۘd?u¦´áÍ:?ï×TîO'? ‰ÚnõÇ?hÔ^Ô3$ˆ?nÿöÓÔW¡?™J‰‡¯©?Ÿ[ØV땢?îcî®T6?œ7'[2b|?4ºRss?ƒ
(ãÃ?¢ÒƆ·?—`å;ˆ%?ïfó1•¬?‡EáÊ?$âb%X‰?0È:4L½?"mÿ×?‡êƒx§3FGL J0847.1+1134@jî4 ½@>à•¿ðExÀ9¾Ñk—þÀ;x}›ö¿î|"eÞ^Î@oS"ºd?û؅_¥×ë?ïÍå=Sj¿Øg½¯ß']¿×ÑåÙkÊ1¿Ð'oO²ß€AGNbll?ïëÕG¡?fÍS(´?NJÔgõ?J—PÂñÙ?ZžëÞ½=§?cN ³ÙÀZ?ïÉk½s?}`¾Ã‡žØ?f›ùh.?jDnpW…ä?p"͕^»?v>yßcd?îÄ*¶5Š?uߨŽ?4®y*?"<KK¬±?—áã ü¹Ÿ?";D[ï&?ï+ï32(?'ÞW­â˜?4"@$'þ7??b	ïrto?š/̙-.Æ?ë¨Þ¾™3FGL J0849.1+6607@bY_í¦a@B8y@]¾!À9Ô"Nßa$À;ØgÕÒ/?ÄíSÜ\H@ä'áqI™@!ŸàZž¿Ú)ÙuÛ,¿á™ ù;Ò¿Ò"¦wgYo¿çáMž™AGNbll?ïõÝ«€??R¦°ÂW?=L¿?@êåìÔ"Ï?IåE!v¼?K–Dû³Ï'?ï˜ôÁxv=?†°<O6{?x-'ÍÞ?u «Kn¦?{Xx>÷Î?€n¥Ä'÷U?ïd{pÆ?ƒçyA]e«?À.§/Qg?{­p"ð×?‡ÉÐDeŒ?{± ¯†h?ïf]Ò˚6?‡GªÉúÐ
?bÁìöG½?aq¨Ž¡?ÜÃ×C?…¿¥4¿¶ß3FGL J0849.3+0458@kÏÿšÏú@<hÿƒ~À9Ùé¿KÛÀ;£Ö™Õ(¼¿Ì¬s"é@CŒxsÚ?ÿƒ3Ù'?ïÙ]KW
пãCUˆPN«¿ÚJ,Qº¿Ý]4wð–DAGNbll?ï¼`¯™w'?÷†&d •?^—p8óú9?`¦Å‡ÎÞÀ?z)Ì%8N?{ªýB5–;?cÜr?¹#ÕmÞ?v^gN–7?}¤<B0"o?}Âg,ûÁ?†	/aÐ?gìÕ?'ÔÉ	]5?YgõÞ?ÁPc!ªÏ?œ!rNjR?‰	È•Àš?íùlTË5b?£¼™7
76?kÒ©<?h½Å­\åW?®·ˆ»)®?£'Ñ
Óþö3FGL J0849.5-2912@o"
ŸS @"vï`¥bÀ9†°>÷Œ"À;":]Éß³?ÙÉü	È£@-Æ	99²@ñ¿€3-¿âw"©Կ㆖O7JÅ¿Ö֙qM¬¿åÿ¥2AGNbcu?îpC"A?©QX¼´0'?o–P녁?r{Ùü·ùw?§¹á­6p?¨
Õß!?ëæœáW½#?»;õFt¼?"d¬Ûöw/?`oôîx?»±í¾Dy?¹‰Ü<ñé?íñYêvUë?›Ý†%Úô?'Y
}ñ±?~^(¨É?¨=Ü¢\?—A«2ä?ìêhó7?ž©6jÛ?ˆ8Þ™Üp?'y)G½h†?µ¥¯+å*¯?œimµÈÏ3FGL J0849.9-3540@pTÀ%@ùJŸ¶i3À8ýJh˜À;9©y
­Ù?äϳ?'@äSV>P@÷«ßla¨¿ã߃<yDZ¿áаd6`d¿èÌÕ÷vw3¿å%¡8/­~AGNbcu?ïÇ\J%½?w@~-
ô?j͓º¿?jB˜W@)9?mÖ"δ" ?oå)ç®.p?í¡¾—ƒ?´]àÀ̦"?s'pþº=?y¼G&‰ÄÒ?±¸äø8<?³§3f}ßâ?î)Ôë'X?–‹Í¢Š8¾?•DbI¿Œ?†ÂE`£j?¤Û1ŒgbG?j§¨R¬?ï&fd¦'?Ë7т޲?a~Ò¾'Lv?bÆuô¾I€?™Yv2ð?L˜)†Q3FGL J0849.9+5108@dóM@$³>@C‹ßœ³*À8…JÿÓ?À;"2¨É¸E?ð;çҌªH@'øyxçÈ@Bsàwy‰¿áJÈ|ÊÅ¥¿ä"W¿â+}Aý®õ¿ìéº~wAGNNLSY1?ïÂN"Ͳt?vPr-?xTAx‡—'?t5T¹e%?Z҂|¸Ã?Tr'Q?ï҅HŸåŒ?y­AÏ?bÕÂý—_?jˏWÜ(b?j¤ôbƒ?qXÀ¤"?í)£$†3Ñ?¤s >~ñ?®$,¹m½w?Ÿ'p¡?{?žƒAü^
ð?Ž¾Ü+±7æ?ïû@ת®?RÏÔ6>ùö6|œ?NÆØY;?B¿L?¡fk?Qåutjã¾3FGL J0850.0+4855@eNù?ò^W@C£ïÿ×¼À8hìt2À;oÓ £äv?êxÛ¯iœ@Æûþ¿ö@vž_|s¿áœej¬¶¿âå0
ö¿åB™OœËR¿ã8íÉéåÚAGNbll@?ïø'QQՊ?Gùú!y…'?=£¦Z8Í ?:€Ì!rä?=ÉÏ۟?AÌÍ É?ïÍòƒ'vú?yÉ]ћd?fv`ºš€?nL¶nBƒ?k—²î†;?q:­?ï;Ù(û?ŠÔžÖªà:?"Ýz´81?.LÔà—?ŒbûIS?€^úéùm?ïê¹p€uª?mŠˆçiy?"^wƒ¦?,öFvd?d$¹˜á?m|×3Ùƒ3FGL J0850.2-1214@mÕ¥€Ãÿ@3‡aÿÏX˜À8#¢á@øÀ;'\Ôm*?öÄxWª‹Ú@C™DµÃ@R‹Ö7"§¿Þ+¹½âŠ_¿âÀûˆLV¿ä¹2X9Io¿èܟEðAGNfsrq?ï韉²–?]?P.¾ú!?ZÅD»Ûx?T"Eú
?QûçV?RJÐzKÙÝ?ïΝ:ӗð?}4bÏ?]¾Þ¤¶V?b¡µ§?qAដÚ<?yV‹ß@5?î=À—½mA?Yùòa?ž!)sš–?"Ґ£?š&ëÞÞ½m?[È+%Íj?ïïñD@Ô?h6wƒìá,?`aÉÿè
?D°Ñe'c?^—qÄÞ\Ò?g{ȏ?03FGL J0850.2+3500@g‹gk*@CBî¤ûÍÀ:—6JÿÀ;÷3I¨Q¿Ñ›>ÎË]@ÁläÚµ™?þ¼òÿçVf¿ë>rH"¿Å¯c)ü˜¿Ï",¹úì¿äÏ$;&OSAGNbll?ïöàOË?ø?Qª7å?G`c^$?M¬‰–&'ý?9ÜÀßD'ˆ?7š
UOþÚ?|]ø?ˆ}p™¿rê?~hÇþ'?zÛ)gÂ?~Uåyҁá?€Ô|¥:ºâ?ï3¿†>?…ÖúU¼eÐ?'Ù'º^–?wW8vrnc?MÛ\
?~±‹!M¿?ïuí¨uNÂ?…ô¼¢•¡?ega¯Ø]Ý?dµ3iŽèŽ?*½v¶8?"Íx,ìI3FGL J0851.8+5531@d>—?·¥ô@Cx†¿¢AßÀ:2)ösDÀ<¢nTqq¿ý<ÒvYùq@ó!i1Fõ@½3@IFE¿ç«—SKà¿àædçn—¿ßI°¹¬ð ¿ìéìPS](AGNbll?ïÅ=Ô:lt?'RÒHm?y,Wh"–ˆ?w¤Çù´¯?PÒùé¾.?O.äŒRv—?ïßLØØG?'ÁæíWÞ½?hµ· êós?l£Hâi«?qÕ}Ãbƒ?~ðòJ@¿?î•"#[?›pÈ3T7@?¤ÇCWî÷B?—dg›ÜQÏ?"^ÆËÁ¥å?"‹äyêõ?ïè´>3så?e:1n¢0? Ë£FŽo?1XH¢®"Ò?fJeW±'?d]Ë{YA3FGL J0852.6-5756@q5X ÕúÀ!ù€	$ÂÀ8иϿÆTÀ;Vóâ»K›?é¹òïÔ6@·÷¨˜@9ùŸ"®ž¿â3ªÏ¡éI¿æaBq>²¿äòŸ¿Îa¢¿æ*í;¾XAGNbcu?ïÙjC*Å?n«µî¶3]?J†·'3C?I»n}UGŸ?oóÂ؍®á?kÌ£r°ìÂ?îJu"`õl?®02(?x[ÑÑÜY?uóëŒ??¨M-˜öm½?«nèd
$j?î¯Ñì†.®?Žš·¡ûö?‹…®G]'?{Ê/:»?œBëK‹[a?†šÛ>M?ï6äÖ1ä?'<ó$êx?`€UÃz¯1?^ª *õÄ?	¬Êmƒ?'õ§Ùô¦83FGL J0852.7-4631e@p§Ü_|gZ¿óº_y5À6£Æðù²À9Ú¯ÿ6¬d?߬÷šU×"@",dŒòl?ÿ6í棿ÝßtDJ‡¹¿äjñER¨¿â²à6áé¿Éx/fŸò#OTHERSNR?³@]ž?²Äk'Á?vÓS±ê±ã?4/æ%p?íqqUPvÜ?³5V,wV?ÜQÈß½–?ՍÙ:j†´?úÅhv?¥H9o§?áòß½ñ?Õ<ɔ.f?ÉiJ†ŒR"?³'m Í9\?®,)'öø?ž?ª·a?çÂí[ÃÌ?´ñ‰5À(?ÙÜwºg?Ãl"gOëÄ?h¹¢{$‹?rF@¦{ät?âù
€uR©?Ãgüå6‹3FGL J0853.0-3654@p2*Ÿ{Zê@ÑÍÀ<ƅÀ9IÏQâJãÀ;C*3<m¿-|ð(@çúU:n@yÀšºV¿Þ[âòí¸¿Þ´<	œX¿ß…±.Ov¿âe `jAGNbcu?î«^ª±?¡Ê,rä
M?uÌ€PdÐ?qɾ´Þ?¢•‡.‹HQ?¡
¨¿ñÂ?ë"¬z/E?½Ñü)í«6?"å6uÕìa?…jNËÁü`?Àa}æ¹ä'?¼ZÃ'É7>?íïGóèg? æÁ
t5­?›¨ˆ}
ð?‰SŠÓwJ‡?°–c¡YR?›SPÉ	Ñ?ìT	"Ò\?˜QM×Zg
?{Q#¸û?r|¦À?»ª¥ˆI¼Û?—Ã«S6Ð3FGL J0854.2+4408@fÀ‡D,@D	e4Ù&À:ô°ÿèÀ<Ü»W?ߚÖÌf0È@íÀÓg?ü󚜲ÿ¿ïþ˜˜s÷?ïí–@ž«§¿³'÷þm¿æô·µ8†"AGNbll?￵ÕîoQ?¦Õ!Í(Ö?wYËϲ¨µ?¦ÇÃû.ËÍ?a–'r+]ý?nÖ&†<?ë³›)&"?Ĺt1ш?º'—B ¼?ÁÞ©ú¤h?ŸW¯'žª¥?¢Ç@:Æ`?îŖœÒ™â?"Ä#©/Ù?'U:
…×?Œ¸ÎT¯p?"÷ñä¢=Ö?ˆÑCÃ'ž?í þ	*qn?±÷4ž½Œ?°¤HŒ˜?°©ÑÛÍ<?'ž9Pößä?ˆ«×¼Ý3FGL J0854.8+2006@iÙÔ?u'@Aèä€G¸üÀ7'tvÊbÀ:ÕaèRdQ?óÙq±s*@ÜÉ܂wi@žåE¿|Ø¿Þ¤Sʋ·¿äL
2n¬¿â.V#Åyi¿å
•Þ½ÕAGNBLL?ïñè|äî?YÖ24¢ó\?3Œ>Æä?/ýT·"M?Wm¡ö"ŸO?Xqf'ú^?ïÕ»çë?v'RíJt?cˆL²T?i2ýÁ˜Ö¿?g?ø­b?m§owlà?ï'qÞ'>ô?ŽØa_Må–?¢Zð!-º?}aÑzû[?'@–ʾ?ˆyj•ûpZ?ïñÄ
ôJ?dH¿õŽ†r>õy†ž"‹#?
qÞô©¥`?\!ÿ՝V?d@ƋØ3FGL J0855.2-0718@ma¿ "_ž@7SÎß̃ÒÀ:º$TÀ;ÅÔî~:?èäÄÛfÃ@ Ì@Šà@…#`,e¿áèyÛ°ŒÈ¿çq÷¦a {¿ë&þ¿ïñۙ2/lAGNbcu?íge?´|Þ\d?£ÜG¼®?§þ«å	t?¥¤éÝrK¦?«xà€+s?዗ѷJº?É·J w?ØOÈzåÑ»?È5íÊÈ?²d†®cN?°ôØZÀ(?ìMûÅÄÔí?£FÝ+£tŠ?«ÙÑ(%†{?–/?º\?¯Fr{*½?™& 3z?Øž´¡#*?º|4*Çâº?ày,šË°?¿‰×Ý\?»È W"Ô?«Œ——"¬3FGL J0856.5+2057@i¿¥_5½@B?l?Ä;.À9²E¯6¹ÐÀ;!¸·l¿ë;¯P @À7·Qex@|Ì¿`Ó¿çéO?Ù¿ãdÞKy¿âkt}UkA¿Ü-I~AGNbll?ï᫾Œ?q¨Û^Šæ?ErvŽvíì?AÎÞ.Ñ?iž·@£·/?pV"óg?ïƶ¡¶Þ?xóŒýߙD?hwÔ'F?g'©å0K'?phÅpcK?rÅõ, D?ï3¹˜1×?‡cóïÉö?À³{_o?q?›¤ôaÊ?'­{î"I?'>‰@\?ï{×®í-?€Sx¦x	™?2O UH?2ž<;â£B?;ÍÏ×Ù,?€C4W
Ò3FGL J0856.7-1105@mÔ¾ Ìÿ"@5}c`!¨ÇÀ8Ku€µÀ;ºßd?ð5`ç÷J¥@Á©Æ˜@gUê¿Úfñ£N'¿àúÑ©Á*¿à>'D´Ý9¿äYìý¼%AGNbll?ïòöêÏ?S›ÀN'ï?E±X Á?BOH½Ìü¯?NtgPh?L8M>ɛ¢?ïÚ
#?œIKÏq_I?kNìt¢?‹¼Uû Ÿa?Žž-÷ŠÊØ?"Ølœ²?°˜‰ô?˜Ø{‹7cË?6ùŠîòv?†«Ï¼TF»?žó-'wHn?"PŸù+cé?êq¡¿"m?­+èKô?£]þ…Lo?™A!¼,?Áaú½£1?«Ž²#ZF3FGL J0858.1-1951@nÊ?þó†@0‹hß½jYÀ9N^¢LƂÀ;€ûŒ3€?æÙq/‡@Äf1¸3ä@³¢ ~e6¿å¼áÀ­bW¿ã8؊ßÜ8¿ê],¿.\<¿átùg=.'AGNbcu?ïòçÓqJ?^¨t¢$@?J0•*ö§?I"pГ'?J3'‡¬à¶?Yº@ïJL'?﹏gÆ>Í?"œ}x¯ƒ?b0d}†Òb?fÙÕà?z Þ0?'l¾™¸ûÜ?ï$ªsʾ?‰3>êxË?"º‰XÂ?y
Cpû?']ÔX…ûÁ?Îxrízœ?o#Êp?†g.ûƒƒ—?\GéÀ%[?`6ÇúX?‹
fÿÁ?…Ž¾œÚ:´3FGL J0858.1-3130@oô/ ê[S@"p@Õ³PÀ:Z­ã×À;Jaοõ5D°^,@â?j¤
¼?û³˜Þ³ª¿â8[¹íª›¿ãyù»Ã:'¿ÝÌ̀i?¤½Üfj:AGNbcu?ï>Ö¥PÁ¿?žä-y,Jx?DŠ³¾B"?HÛ¯Ø'†?—€ÚðIÖ5?ž¦aö#‡?îanô°úõ?³àÿ
ª?j5'W¶?ruª '"l?¨Gí\ÊÕT?³k‡>-´¿?íý—‹Læ?ššŠëˆU?Œú}è¦s+?yûˆËE3ó?¨ççÔÁ"Á?—a6º
œ?ï§åËÕÑ@?•€•Y«b>ó
Ï:;Ó?FSúÆZ?…ý"?"tòM(3FGL J0859.1+6219@c%°_®¼A@C?'à°«À:RV	!òÀ<wJº8v¿íÒ=؆G@àc¶Þ£å@u‡_…K¯¿âÛ]ë‡fÖ¿ìąz¶?¿Æ>ôff3¿êÔeè´ÒAGNbll?ïÙ]±Â]J?qÎtÅÿ$ç?S¹"zr×?Qâ#SÞ#Ä?lŽi±¹?o¨Ü8}U2?ï0x-u?·ßq%ʯ?uÍ0œ[Ï?uVn
wÕ?{š»¿Ìél?Š½A´P5x?íùà#xÕÕ?ži• ÿ"Ø?"8ê^îç¼?ˆ‡6z^,?¦Eˆ˜û.ð?˜«°¶r?â'n?"4'"Ðjq?;ç­á[TÉ?C^'ðnõ?Š½Š«Iz?ƒßIûUk™3FGL J0902.4+2050@iÕ³ S\ž@Báj@ºˆÀ9Ñy÷ÜÀ;w˜³ÀŒM?ãjñÎÂxé@~<)Ñàˆ@Б_äA3¿Ô	V'
¿àDÚõ{äõ¿â
C	÷Æ¿áhCÄ×OAGNbll?ïú'çÙ´>?I×9n?0Ÿ|+½y?*‡
M˜?>!E¡y?GÁWYmd?ï¹r
dŠÁ?}^‡'j?o§¦ZË^®?pèå$Úùo?ss' TðC?vô–€@Ùc?ï2­Ü<{?‰5?ڂXO?"D*Ž+¹ž?{ٕßZ]d?^bµ'g?'À˜HûV®?ï/¶Ró`i?'kӐžu°?jHÙjùÜf?fȒAE«(?–Àt4·P?Ø6Êk""3FGL J0903.1+4649@e¢£¿ø¨ô@DÊ:?–îÄÀ:ªÐ"£À;þ>Ëí©¼ÀÈô>«·S@b{üû"@ꀿƒ
;¿å̪*éì ¿ê§B5sn&¿×ÏE%V¯B¿ïú´ù¾¿»AGNfsrq?߱Ç?©ýúTå?mÀŠ*õÒ?•NocXÌ?'·âeˆÐ ?ŸÁŽÌdRg?ï¹Ùg›æl?…Bb'Ž?n&
—æM?t•Ç%¢?tFæW4?žY÷Ø·x?í­K__ú?kV¤? 6I¦9?'öí>}ä?¤ôÍqZ?"ΰ»@¬?ïÓΖہS?€ö	dƒ?!/Pÿ¨?E¿î¸}r´?u¬/ÕÎ?žŒDBó3FGL J0904.3+4240@fSÔà—"ì@Dña_–hÀ9øE~RÀ;åٚ:©I?و]·k;¸@j3óL"W@ο¿É?¿Ý2`Ov
¿ë¬Bn~¿áàʐÀW¿ãÖ–íAGNbcu?ïÕ`¸¹—$?vb¨È˜û?Sò°¬º¢í?W ©ú®ð.?pR÷xÅ*?s HUM #?ï9ézAS?•^Üâ?Œíž,½\?6nuí?"—ýô²?…"gg[Üë?ÍS?3«I)?Š3
σҞ?}ùü˜C?›æGÖ¤l/?…>TáDo?î@+_Žw?žKÔO4°ƒ?ŒÞV3øÖ?…#b¾0QZ?¤ÅȸÊg?›pÆ¿lS3FGL J0904.8-5734@qA¬à2ÛÀ! ßÞøHÀ8W,ˆõ¨À;.Ãø贊ÀBjØf@Tꙇ¸@›ÀSu¿æë!{r3œ¿â<>.äÄæ¿ãëË'(Ù¿ÞÿM»8êAGNbcu?ïõU¸è=?SlöY?+`Ñøj?0~÷ě?QòÂFÌþ?Q0*Ô¬B?îýxý³MÎ?®íZÈ¡?i8§û~?u£0逴?)Ý´–Ö…?¬Ó䑤[?î6Ê%"D?™l.O@?'P݊žŠ&?†E*8í?£êî萶­?"•(‹³µJ?│g??~a	èk>ö*¿Æÿ¾%?!ñ_öƒ#m?€
åÆWp¿?~]v—Ý3FGL J0904.8-3516@p7߬£b@R ß´+À8¤ÌHBŽñÀ;NÞ̀Pó?çB4E,@Ž )֓@4TçÑá¿ä]ÅÀ¾÷w¿èQKòœÀ¿è	YQnÌU¿ëÉvBÉˈAGNbcu?ïÛcÙ%™Æ?lËMóqû²?Xám?÷–?SÒ™äHò?h+p:jyn?h€TÜp!?î^ۋàÄ?ªÀo^ã·)?vøF-Žòƒ?x­ý'8?§3>|Aà§?©{3:ß;?î?\,Ë?•pH³ÿ™ñ?˜!¢÷J@Æ?ˆâmŸ¦?ŸòÜ3åÙ?Œkñ@O?ϥÙú?šxW‰´C?vß>úãU?sõžùEO?¡û[&Eÿ¯?™RåËia3FGL J0904.9+2739@hÎrà\̊@DE À:W%ô†O:À;å)äÕØ¿øĦf%Ï@
);}"@DßX¿¿èfŸ=ò2¿êqȜçVç¿à4>&}Ô¿æØÿsú3ôAGNfsrq?ïڐ¨Q·Ú?zÎuQu´"?E@	Ó­x~?LÅîx(6t?pªœ®cy?y`JùG·5?ï–öú¹…?"3PC'%ï?vt¦$ó7?€ª!'‡öp?~Jݯ­á?'âº;ƒ6?î8Ý0¤©v?–0ç"Cõ‡?ŒÔåËZ¬?€½µN*±8?¥<ó'ÞæÉ?'®p&<?ï†÷'îD?ƒOixÿlï?:K€'?BhíœB?m¡CÒï?'Þ`v'â3FGL J0905.5+1358@jàÓ`Ð$p@AúQßƤ•À9öŸ..À;B̺XV¿Ç½úÏñ@"gtƒ_›?ýknî1÷?Á‹á.Gà¿Ü¼pá6Æ¿Ýĺ]€¿Ôš:YÔBôAGNbll?ï¸a#?U?}Föuyç?gnÇM
Ó?e	Ê¡æ8¥?x
¹ñÆ}?xŒÉìQ~?ﶈÕæV}?€"yõ/¨?melp†üR?jϦ?Ii?vÞԑCd?|z²êÞ?îm$'¢?"rxKÊY?'Û°ÒÚ[?…º×ĕU¾?D¼ØåE?‹û貙	?îќÓÂ?™ô4@§?byª?¡Ù?cë9Á2"?®›K›¸«±?˜¯³Ÿf3FGL J0906.3-0906@mËýàÖo
@8• ŽÀ9l'^;õzÀ;ƒ0"'¿ÀõTͯR@-Ñ4§@, šTU¿Öø±*"¿âû/–pšG¿ßi²·#¿ß:*šÐbAGNbll?ïßï)7?iôXøÀ˜|?RëÎðíž?L|ë¾Œ?gn)‡Íџ?f^›&àÜÿ?ï¸
ƒ™Ø?螗–N?lP¸¼‹Ò?k½ï'á¶?uÐâ) ÍÛ?z?:`&$ñ?ï"I*?‰¶CY?"$?ˆ|k gÀ‡?~/;`ß©"?"QG檤?qu{Š˜e?îð—HÞ-£?'C
WØm?U®©ú]?Taª*µU­? I&…þ?Ì<iH3FGL J0908.4-4916@pä˜à†8¿ñ(Hÿ"_{À8r.ÎI¤À:VZ°O¾"?ä³m»@ÚÍÉwê@"]60¿¿é'íø…Q¿ç׋—£J¿é÷a¿Þõ^®XÛPSRPSR?×=ô[³Ž?Ìò'Û|CB?°Ý?£…ˆS?±là‡$i?âEÐau/?Îý.D<3ç?»Yð;†Ä?Å£RñÈÎ?´WgìýÖ?¼F:«"í?ê	Ôú?ÉEgHˆŠÚ?Ðó°å>1?±óÍm?ÆZ<¢ý|ß?±±¾¯´¹?áï˜dy¯?·»T"Ýö•?ՃãJ³3?Á@=pXñê?—<…–3?˜ãԏ¼4–?ä…VYyµ?Á‰n
}j63FGL J0909.0+2310@iŽŸ¾vÉ@Cö?µ!µÀ9š@€MÀ;`¹4i"¿ü
½áÍe@*ÏÝMy?û`àÀt¥¿å¥<Ê¿ä9÷;D"¿ª¹;9UÐÜ¿Ônô'¥AGNbll?ïýÂúÝ?: ¹Þ,"?!ߣ?ì$/H·?4û–f·}?9~|É7Ì?ïÑ'ðŠnS?}dÒ¯äj?cdÞMâŽ?j`u‰ž¡?k¹ª—CÈí?v­mrLÅ?ïãaò}4?I' lÎ?s¬âÀÄB?sÊFÎ}—?…±Pª?{¬"ëû?ï净CbZ?gXÙÖ±s>±tº%¥Õ>ÀºlGž?jv\Îa
?gWÔÛü¶]3FGL J0909.1+0121@lžj_"ÊÕ@>íÏ ¼£ŠÀ7Ø:ø‰À:Ì;ëh™?üj%
%É@uÔÔÙ
É@AÔÜ:Óæ¿ã'xµ•Åò¿æ–èžÜÆâ¿åFi÷óö¿î5 é¼iAGNfsrq?ïHÌ0ié"?"#i/̼?'e:å‹|n?ü;ùšÐ ?rü4ÝCX?uÙ®"¡U?ï±Å‰¡4è?''´ž) ?q8Wÿ>FÍ?tÝxö³;?uäã0'EÁ?xlÈû—œ?ë;=%+ÝO?©J[ùÉ?µÞ2&ž*ƒ?¢7zRÓ&‰?°Gä°ë? /¥¢Öɳ?4$n?¢f6Y?|µ¾"'Ö?‰È|~Íæ?¢=z¥ç"2?Ÿ›*}¶ø3FGL J0909.6+0157@l_ 'á@?W°?ÎL)À8û̈Ú.µÀ:îÁðи?ÙÅc@0
¤@wœÄœR@T/ŸªÕ¬¿×ÀÁ`¤Ó¿è¡ ¹*zõ¿ãOÿô¹È0¿ïþÎSNusAGNbll?î£%‹͎?§™|VW"ƒ?vîäŠ>?†Ä£`7'è?¢ïʽ‹fŽ?¦…àÁ\º7?îÝ·å"‹?™äϹ?•¢!«F?'¶SW뉴?u2W†?íÇbºÕ?ç¸GÎË@D?±T/ë•<p?µ^q†Ë‰? 2A&»Ïÿ?Æo™™*?®Âæ_üË%?åÃ
	X?²—~¯r'?®
Æ¼mÆ?¡;ãô5'ë?и"3ÂB?°â#z͜‹3FGL J0909.8-0229@m9pޏ@=ìð{(À8Æ,p¡RËÀ;ƒ†.'ÊJ?øA¡^›@ŽßZn
 @"•úR¿ׯ"[ê¿å9Z£æa¿ãÏý‹RüI¿î'´m–—˜AGNfsrq?ï]Z<'â?'š]ۂ+?Z8ÞJüå?\C4PÔÈ?oÔ0Ñ7?s~¯A(âù?íMZËk¬0?¶iÃy
5¾?®€ÒÓ½?´b¿"ÃèÅ?šK¦ˆäÒY?œ¼""7NQ?ç èãH?²5BÑ2ZÄ?ÈÿÎ_ô?­©™ƒÜ(i?µØײÿª?¢H Ò?ë@'}ŠIq?±*ò‰XTÞ?¶(—nGøó?«È%p™P[?¯¥©JËw?¨F/ÁuØý3FGL J0910.5+3329@gã×@Än@E:íàBËWÀ9!þW‰TÀ;T4£u»n¿×,If»4@oÀ£ÉžD?ÿ¿/ •A?ßàÜn€fB¿åwuÂÏÈÖ¿Ý1i¿Øτ!¸6"AGNbll?ïñ¢Ÿ9YB?c"¨x?8@hbGvO?EÛWA«Ñì?Vª§t»¡æ?]Ð/möñ~?ïÈ& Ôöö?yÆ<%ßm?keh,2!í?oÿ©"Rà?ltvþÖæy?p`$Z¼?îð҃í'?'p,'–†?'ï
tl°f?€6
Z>«E?˜n*e«õ³?}ÐIAþV?ﶅðX×?'éç§Vs?Amaà?E˜sê±?›À§.‰Ö(?'ÄÚ;å3FGL J0910.7+3858@fö@ÈG,@EÈ?ŸR@À:á6U&£À<]\Òhî?Á8Tú3@Vöï‹Ã?þè`§	Å¿àò
·'$?²'Ÿ¾2…¿áø@{+¿ÌhØÞ VDAGNbll?ïʘ†'aØ?†ŸÑКç?p·›õt¯?vÎ7À>)È?e2
 ³?]?ƒÒÜ&Ðen?ïŠkqÁÜë?¿qef·?€ål?ˆŽFYU'?z¾F°"?€ž<Ð?î¥Î""[?"¡=G'¤}?"Íô–È~?‹î–ãè®?—x9¸ßÌ?†t5*ä7?ïV­äl‹?#ÞÔ9ìK?¶
s¤Å{?":fi?ˆžyqXWù?'ÿòÍِ3FGL J0910.9+2248@i¢Ÿ<pÊ@DƒڐÛÀ9'4èÀ;—;-C/?â=€á^K²@ŠT‰š"@É eϿ׋ͮt2¿ãtÂ6ñ®®¿çuᚌž¿ë_[XÑAGNfsrq?ïï(ý³"?ŽˆR^Hç?‰—Dýüw>?S¶Éºª?Wg†µ™?Y?l'Ý#†?ïÁ<Üëçº?|‰÷Îoûž?kÍ
x-?nj»yìdw?q{…fª?tZ{Ë`?ìàÅJ°‰?£3mÐÓóB?±'4ðE¸Ñ? ¹nâ(X±?ŸJ'è×êð?–²/rf?ïžÎ?¼?ƒ^¡ZÆ?À?b^õ͂Ò?c8ÿºá?ƒáü°I¶?'<W¯æ43FGL J0911.8+3351@gÕ¦°)(@Ec—tüÀ:7‹dL°³À;™¤µVŽ'¿Ý/¬	Lž®@
bmÔï°ý@Ììš"ì¿î7á…ä¿«ÈMÙt¿à
_¿O®¿×ÏI_«cAGNbll?ïã[IpWY?u(ßE	?Jr\˜ì—?GjéÝ"îÀ?fim£?sÈÿD‰ Ý?ï¹aÒc»?€'†]›8?p" ÷kÇÖ?sæåØÁS?rÊu×Û?tÏðoêu?ï†E#4T?†!m!Ü»Ø?ƒÙ›#z9?uÀù:3?''iÉÜXé?€9BŽEÎ?ïf­z•Å?"E32Sw ?\Ã׿ۙO?\`tÅy"Ê?'^4Ï?ƒiO–tŠ3FGL J0912.2+4126@fŠ¿ðEx@E«³ß•ý-À:_›q
.À;ÛßÞèX¿ÍÐU5¼@
:MXÎM@Ч ¿ê™'Îr‹°¿æ	7ÖÓXO¿èÕ5Ú"©?–sáÏwQAGNfsrq?ïã(͍à?­å¡pÏ?cBŸI·u"?£ÈÌbƉ"?StoÑuSö?"r¯§Z·?ïÏdèók¸?wp{,ôq?eÚ¹ÈÈì?j?㛑÷?jÀ]CÌ8Ú?o"µ
ÒXN?ï˜6
ÜëT?wÐ$FQŸÔ?rˆNˆêñµ?lf0»Ð?€®UDO²f?q̆äÇ.®?ïïpóGæ?bKÏ~›ãÔ?5,`A?=îz"ß\?`28˜ås?bJþâ¦È3FGL J0912.2-6452@q£˜¿pÀ&~wÁ½oÀ:
ÑÒÆÀ;­QU])§?Ú±¿ë³@Óá:(@tߥíe¿ädùŸÕE¿êÐKÝN¿Ü|í¼[u¿êÏœ'r^OTHERglc?ïBŒ=Fª?£²ô5ÔÂü?oÿ±Ž?rÙ:Íåa'?™U.'4ù<?¢á‹x֔?íNË÷M€?´60¥°Ê?•´e	¤d?š>Õ­ºÈ?°‡*æj?±UµÈ±N?íø1†/%·?—L%™§
?œ¬)oV>?‹ZÂJ3|?¢mˆUù~?ŽúSú›?íD'«Ÿ7?¡µ‡Qù3?Š°™àö?"Tª.0è?´cÊ'?ŸÇ´æÌ3FGL J0912.4+2800@hÐ_ôö@DðãõhÍÀ:sḻôÚÀ;¥Á*[J?êpl÷м@¼™£Õˆ?ø¤¨¡s3?ïýð'
g¿å#º'ê»Ü¿ã!W:é?Übö¨œAGNbll?ïÒ¥•<Ì?}žvújƒ?V?žQòc?\`"R£Ü?qMÍy™¬?{ Ë*à'?ﺶGòÑÊ?aà=©di?r‡¦¨³?šöl¶°"?pK_îfß?t§'9'cH?î7Uiä?œÛC¦ý?œ™‡8w`o?'ê[+UM?œ{ˋÐ?'`©¹c'ý?ïF]Uw­í?›î´±¡-?[ßë-à;ö?q‰¹眡?•vVž,>À?›F£h£¹3FGL J0912.6-2757@oß<`Ÿ@+×n Ç‹DÀ9Ì(—ξÀ;—A<á?àÍåù;=@ƒhÄÍ$@"ö`o"¿êI:Û
$¿è–™*ø•í¿âV¬ƒ~¿Ýºfá¾ÿãAGNbcu?ï¾_S0Û?™Ñ'.3C¿?\Š"áøæ?mÃGŠ€]?y­Í¯lé?–f•ýOË?î·½íɈ?®\š;ï»E?…7å!•¢R?úŠñs?žliq{ýÆ?©º*TkT†?î‡)3<à8?—Ú 9[_?‡dó£™›?xAà˜`®?¡´/ãK¸i?"÷4	ù¯Ú?íˇ'Sþ&?¡ˆ"<V!?ƒôóB	)7?ƒú\[\?®JPº=ÓH? OÝ:²qô3FGL J0912.7+1556@j³|€"Þ@C)è°ºHÀ:dÛé*ÑÀ;><{±Q?ÛÐ?фË	@ïK"é!?õœkþÖµ.?䧸ò¿åÍY(¿ä¤ÖFE¶?æ«9åUAGNbll?ᅲK§µ2?†jd>ñ–Q?@!B©g!y?C8/ƒÅ·Ô?~01Öø'³?†]ÿ>…ž†?ïÌàsKÑÎ?}@îè<ó?eÍpYš?odÌ?mR‰CԘ»?t†>·¢#ø?í•gÞâË?¡Îºã
އ?¤ˆ…õ")?›C'…,‡?¢ ü*-Ä2?™I†Þø|?ïžÆ€vD?'u÷ùz›?/iûŠ®¹ ?NU{óš}?‡Ð·ôD=f?'\Ê%#ã3FGL J0912.9-2104@o3b¯È°@2zeÀN9IÀ9.66òÀ;Uv<?A¿×Í.E|z¿@«%󄜇?ÿä~ð ¿ã°ïÄsŒë¿àõíSļø¿Øõ@gô¿à¨&¿AGNbll?ï՟'É¡Ã?u6°[(ø?IûÊ9¾q?BF"‹3J~?qðÅS÷J'?tÝFu17?@…¨ƒ?‡'¼_´_‹?mp?ˆÛÅ?lðàPŸ T?©§gP=?"y%ñ="é?îÌOeˆT?7}0SgC?‰€Z4 Tã?,:N.{?™¼høþË?ˆùÀ	̝?îIb—
•?"¥ø˜:?SÐ?ûUSS?T‰ß¹¼æ?ªËTL@?"R8Ò÷3FGL J0915.0+5844@cŸVŸI@D¬à f§ÕÀ:®…à19À<%çbzH›¿íªf@%ßã@ÄÊ7J3@ڝ`˜¿ä%Š9eŽ¿Þ$Žq¿­L¿ë†k‰2e¥¿á錐òAGNbcu?봀áÜþ^?Ê3ÂV<?ÀíWÍM,?Êáj•?`)]ï®Uq?e{þª
Ñ?ï´-$ÀˆÌ?†¹ ØÉÕ*?s ¸ÅŸüy?{¥÷wåÅ?rȴڝþ?x
é|Ëÿ?íYƒ^º³?¦…7°Ó ?¬‹¦¤§?¤Œ=~ùŸ¢?œ"|ÛtB?ˆ™Í¬lô¨?ïĄVä?w!{ï½?T/b?]ÑÆO£?x²*"™Æ?u5€ÖþÊ3FGL J0915.8+2933@h"žà*w£@Ewa_–hÀ8yœÇ]!À;ãÙq÷¿ÕF¾1­«@!B"ãÒ?þFA,ðú¿ÜÙ{ÞêþÞ¿Ûçª\-2¿Þ{å†#'y¿×+jš8âAGNbll?ïƚ?ü¾ü?v¶íH?ah€Ó²âx?_¥SäŽ-Y?sþŸ—ǘ?rY-À¥"?ï°h\œ!«?$ÇxôY?sۚâæc?t2WÑ3Ò?sð6ÏéC–?vm‡ÉÇèO?îBYÏþ§?—ûý%Ã?'éuß?"{ìÀ?£M`ŽE"?'q‰íp?íxQç5O?¡Ù"rŠ;?fÀº–ªƒè?iàî1¨"¯?³…wœf?¡‹¥Ãä3FGL J0916.3+3857@fø{€©Þ‹@FÁ?À:qGZ1¤¾À;ð¨á59ž?ádû3ßÍÓ@ZáZxq@Ùhy?í[éTlê¿ã¾grJ~¿êÃa›³¿â~¨ÜŽAGNfsrq?ﴕֶîÕ?ˆaN ÝE?†¥&'È?‡,ŠéU?Lð:Ñ܁{?V>""'ǟ?ïD´¯L8?ž(ã7?öñ…º°?™Nn¿ê1
?¹Ý;l@Ò?"=–f†Y±?îÖ¢÷*?!AGً#?¡*~æÉÇ«?—R	/?šÐ-Ӈ0¬?ˆA‰ôgÀK?ì~6öáè?³=ĸåV¾?²°ï¯™&q?®ß¬€¶"?©6=1_"¢?¨n]‡`à23FGL J0917.3-0344@mfˆ_Js@=äÀ_×,À:d7EçjÞÀ;²ȼœÔ¿ïµbXBiå@mó‹R"?ü7ë¿+N¿é8}RÈO¿×9[B"Dã¿ã–>¢@öÚ?¶ºÚM
AGNbcu?ïôD啍a?Uš·Êt[Î?6NƒFœO?4À¾µòÝå?Qâ">×?S^Ù³õg?ïÏsùA?{Ê»¼ ê?aݒÊöý²?gãn#2t?n¯YÁu?tÂ,Y©n?ï8yu¡à4?…ƒ¡!þ?…üz	ä'ä?}l®Æûùu?‹å(£a?x|`B?ïØÀÔ^Þ?q«pË*ì?Õ¹8Å?̕f0)?sr£Ì!/?pý¨]ye3FGL J0920.9+4442@eö*?K@Fg€iFëÀ7ƒLŒ ŒÓÀ;6K\äÈ?üÏ͍'ùg@â$Læc@ž–Íar6¿àÎ"Ž[‰$¿å0ðÎ3Õ¿æôc6'§¿êUYyK£öAGNfsrq?ïØô¾0½È?j›BÑS‡?o€tæ(?iM¹ú›¢D?N+6Åp?u?H‹v³³EÄ?ïÖ.'üP?wÈRwof?c`Ý\›µ?k\·7Ð,?fqgûô?oÖÊ¿&µÕ?íwì+–?¥Óü±Ó'?¬à»îõ3?¢it_?—AÃ;U7?'¬–ÔÐ?ïøð)Çß?^ýzâü?fR×Z™ÿ?$•2ÊÏ÷:?JØó³R¦?]¥a¿Ø/?3FGL J0921.0-2258@oŒ¨€QÉ÷@2¥`À:Í~	ZõÀ;ÐNË?.?ðVGšs^G@Òܚu6¹?øÙì€nF¿îØ]Ø´s¿ïÿY<ÛÞ?ïÿd3Rµ&?‹VD"ÍéAGNbcu?ïÂULž(ñ?Œ—©K9a?Kp¹¢
À?X"¨@f?{gEù·Ev?‹i$zqB?ïUæ'üÌ?²™÷íÈ1?oGÀ²QÈû?zî±ßl6?'Z5ä¶-k?²%#÷֔!?ìõ_™ð?¤CHFãø?¢·ö"U³?–£»#?­òçjjù?ž»A£ÍJ?ï>!ŒmÉÚ?¢QÞ é¾÷?4ð`‡J×?ZQGÀYÿÐ?—èð*{£?¢T£³#ç3FGL J0921.8+6215@cúâ~@D'¿ó vÀ8݂ßBñÀ;ÏùrGE9?çþRåÄÚ)@ñÚbâx[@–sßË­¿âxõ7'«Ê¿æÀ¯e2ߦ¿å4eè'%1¿ê
,ZÉGAGNfsrq?ïñ–Ç/g?`ÇÝóš¾?K¸Ç|²G?R‡\™€?MìÇo³"?WIÝ:œ?ï­ÖT*Ñu?'—ŽÞâVO?tb£õÝ.?u:ˏùM‹?t²1ôº.5?x"*¬gÃu?ï8Éÿû/|?‡va.;0?ƒu̼¥ç?~=ð:È\ž?ŽXy4wzþ?‡D8îÔN?ï ÛÒïw?‡~^›sê?h6a¯|…´?eÐÖG߄?»rØ_€—?…ÌØeb\3FGL J0922.4-0529@m¶<ßï¿@@=èKŸ:ÃJÀ9°)3ÕðbÀ;±m'ª'?¸djÛ£@£ûùá@Y ÿ~û´¿ä&B×7¿×§¨%"¤¿ãÃÍZøZ¿âÏ1,·‡ÛAGNfsrq?ïîh"Ä2ù?_y"Ôq??'>‹+?:M©dZãþ?[O9¨gP?\*ŗ#?ï®Ù(;%Ä?'©Â—~?q¨ÓïÒ¯?oæ7"À•?vê—òßK$?{UÓ®gU˜?ïUÔëv¨Ì?†0cg{r?'Fò˜(ô?}OGfèÁ÷?ˆCҊT¤
?}\c¹}\?ï;MpÕ!t?‰`}~ŒÏ?p¦£OÃÅó?h?ièèå¸?"l©jà/?ˆ@öÑãs3FGL J0922.8-3959@p•É 'RT@ѿÀ9ŽaêÖ£À;n©›o\¯¿ð`ëeU@8¶*@žlŸ~"¿ë@†NÒ寿ãÃ¥×?—p¿ëõØùù"8¿]Í­"Å–ÅAGNbcu?ïÐ4[9ò?v#YÖB
/?j҄µI'?møZ¿dÒË?e(Fï||?g' –ªÎÊ?îk5úï±7?°b‰wh±Ï?lˆ%D~•?tÜí«	‰©?§"ÿ@¤'?¯×LsÕ8º?íÕ	"^݋?› ꮺ"?•m»%¾?…–©²Ù?§ø‰."x?–eË÷H!?ï¡SߖŒ¨?«Fˆv"?j­÷ø¦´?&µÊ«Ëw?‡z2¾lä½?¡XA–H3FGL J0923.1+3853@füÜ@W@F´ a3÷À9Ï¥ôïpÀ;Ðbƒ'Öß?×â
ˆçg$@:–n*@,À'wé¿ê¦×>ã!¿æ±ÁäÄíP'•
¶	¿ïþiWVAGNbcu?ïø¯›1rš?K™d«U\?@´¦–qlX?>f©JÖÄ?9ÙGˆXk?Bf^•¥<¸?î‡Â†Äì?£Î:ä_¹?Ÿ"Š¼«? ø~`ò?Žé5:
?Ž¢ åŒY\?ïA~G´Y?‡ e7#n´?‡¨ÇͅÀ?|é%u…QM?‡÷¦lÍÛ?~‰4ª$Y?멝йµ$?¯ýÐúIÁæ?¸ô<Íê²?­Hè¼,A?£}©XžT?›HžÔ^ù3FGL J0923.3+4127@f‡Ù!…Æ@F·>À//˜À9cöHòÀ;ȉ¬¼Œ?ßϙ'2@äNô"Í@	3€
&u¿Ü'èJñY¹¿ä–'˜ôX,¿äèZÄFÁ¿ä¬£b¬XÊAGNfsrq?ïðÐ]ws?VDJ|äá?J¯rÔõ?G[{
zã?Rt¥Ûžü?På&±`ÎS?ï¬åDµM;?'§•iS0?v˜¼«rG?x°ä&_ÕM?rô ùç`?u-Káí?ï:Lóç?"9Ú°	Îc?ƒ9S¡^9ª?vè¤(ø
?Ž3ª[dÌW?{á'Hp?ïgúE(‡€?‹ê:ª?oçÿƒsQÅ?gÀîú»ó?ŽnÕK©?Œ3PFw¤Ú3FGL J0924.0+2816@hÛZÀ?ö@F7¿Ý/ñÀ9Æúû´@åÀ;àÂ=&Ò¿êƒ
^Ü7@LÒõÛ¹Ð@^`§"¿å³|ZÍ	¿èÁ­cÈHÑ¿äV&²h¿Ô¿ä™°…™\ˆAGNfsrq?ïý.CH¦	?:ÍãkÇ?Ý:J{?ó…°ï"2?1&n[ "?6%ÍâÖd?ïÔ,ôv"?vçBÙï¼}?e
˜^xôÏ?kvÒc,å?fÖ:­wÚ?mø"Ó7²t?ï‡Ùióú?y¢QŽæÐà?nxŠ÷×?`C+êqYS?†k'ûB½?vV½_,TØ?ïõ]°k"l?Wçi¦Ó;>ò9ÿcI>>úëê½z[?Tû·+Lï?WÇgD•0ù3FGL J0924.2+0534@l\
á'6@B'"à4êÀ9ߔãQsÀ;¼Tdc¿¶¸¤®c@,ÁL#å@q·€	z¨¿âwˆ¦Ç¿í3m³À>ý¿½Ç¡Р¿Ø~.ð"ŽSAGNbll?ïÇ!Ò¼Áæ?'§÷‡ây?6¤™ €…?AB´ª!,?{Í—¥?'4Iÿz¹?ï»Í?ʧ?…²¢õ–f¼?l›0ð°l/?sh''*?sËÇ¢TGõ?}ƒ6{1w?îÄÚßû?'9mÎØV¾?WúÉ?B?pCÍ÷¸Dy?ŸŽ¾)ðÛ?¼.Á0É?ï'õ8—Q?‡+…NñŽ?4=ºÁ?B·óx&N'?Ž ÂˆÖ¾?‡€†9/Ù3FGL J0925.6+5959@cZV`^åi@Eu@ýAÀ:¢,nóÓ¢À;öÓ)ÞÛ?¾']Ç»"@PûSóÈ?úq™ O–@¿ïÿ½Îc?ïù\•W?­¿Ô¯$Æ3¿ÉÝTâãîAGNbll?ïùáÂ͑?Díïɵ`t?: yCL^?@r-–<Û?6ÑØ40Ã?1L|·?ï«¥ÉNR?*é+1~?w"Ï»Üd^?˜¨Š2þ?s
KÀ|r'?vŸgMªuF?ïbTk›U?ˆÎyWg‹?€JÚavOc?u¥i®G{¯?‡ "¢Û8?všn¬T&<?ïƨùî*?yiؤ‰?iNEÖÚ!Ù?j»°Õì4Ñ?p`M›ÚO?t2F¶"–3FGL J0925.7+3129@hO8`™Ë@F«×à&EåÀ:å? §?uÀ<"6;%oü¿ÄXI÷RÕ@9.oÜ?ÿõ÷áMR¿ßù¥»ïb'¿ç>¥Ã¯¨á¿ºø
é˜é¿æÍXðýAGNbll?ï¹(s†z?Œé×80­Ç?bõ칟Œ«?}Êê`è?yõuilý?ˆ›þ
 Ø?ï«Rû,¼?…øa«V?w6±Ÿ»Ýf?ÕP§Ë?sH$â­Ä[?trWˆ˜Á?î iþaâ?•$¼s	ÎÞ?"§¾¸ñ?™
Kôˆn?˜K¥- Jé?†ÜoOÆ~?ï°Åªž¹›?$vH ?A¡¿‡°?EŸû(ø/?'´yfy
?~³Zôô3FGL J0926.3+5409@dM…@FA-@F	Øà†8À:°ÄŸá§À<'ªoª²Ç¿Ü¿¡26«Z@À§8¾o@£¿bV¿Ö[A?÷x¿åuœ#âˆK¿ß2̜ț¿ä÷)攅DAGNbll?ïÞ#šh€?rœAªí?aVJ
 Ä?l£u۞rë?`†Šg^¤?`Î$š`‹?ï¼M6ë|?~³Öþm…«?p(O²IHP?s¼kõi?q±Ø'y?s&¬˜"Ï{?îî×JÍ^?'ZôКEÄ?'áô;%p?'…•Äw}?Žˆ%dF²?|k-)Ãà?ïÀv £—¥?x)J3"S'?BT"
ʬú?A.Pc.?}z],z×£?w<»*`Ö¦3FGL J0927.9-2037@ovýç!@5kjК¸À9 ~¶¿DNÀ;»Ý:ZM?ݗ¿.©‹ª@çk›¦ÿ@ìßfØQ¿Ý@º–z'¿çVá®ä¸¿æþš­ÉZ¿æ¿þ½à ¿AGNfsrq?ïøkžSª?FøRßéhì?7-öêsÊ?5B"'ˆ5ñ?B¼öwy?Bàḭkà?ïÂj@€à‡?og~4%i?eæÔ'W?ge"âS?s×u±üþ?~?æ.ƒñ?ïCîÏÂX?<êÏq' ?'C æ€Ù?u>F¿øç?@«(é9?wwì'A?ï»ç:ÈÞì?~ô6¸V?C̹eoâ?D‰£ ®´?'ËnâÑ?~/澒3FGL J0928.5+4048@f¤4?¢­?@G5Ôÿ¡5oÀ:¦xmÏç4À;ø˜‡Jâ|¿¬»t3Ž<@
y$nŸDÿ?ýz¹>ÐuN?æèæ˜ðI¿Ìú\ßÌPH¿á+9/²±T¿ÄÔ+j*ÚäAGNbll?ïӔõ¢˜Ï?xñîÆ?a·œÜcJ\?c9ŸÔ/+>?j³mæ??t]H=ÔÑ?ïÀ#Q'•1?
OiÚÚ?q(̇ûRé?z/d=O2?m‹]t*b?q 6ÌrÈK?îÆ؅F±?±Æ•ù×?'íw¾'Í?ƒ"â'ÍÉ?•7w ¥\à?'ì"´È'?ï‡)TVõ‹?‰/3ãó¬8?bÉ{œ
?g0]*¹ªš?‰'8‹õã?‡w!´ÿ^å3FGL J0928.7+7300@akO¿ÆT
@Bwa_–hÀ:z²YƒÿÔÀ<
Մ+sK?ä\PZáM@
¨œÕä"ª@T¼ù›¿îeó%•Õ"¿ÚR#îò''¿ã'Å&W$¿éOÆD{
AGNbcu?îö*ßMëÁ?¡u™)ã?™ýrH÷¢?žpû境?|ôÇ5.ò?Š´ß•¶iß?íVâ?²¼ùŒd©"?­2ƒ5¨Ì?¬'àñ•C¨?š×¸xlԝ?ŸÌ.tHû1?íCÚç'˜?¢béß?¥¨Þ`^xÇ?š!Ž€6-?¦s'
¢?"Ë*`Gl?ê½3k€?³#ä‹wå?Àú['?°??£¸ùfió? Eé¨ßF3FGL J0928.9-3530@ppŸS @&xwàâ-‡À9Yp×ÙpIÀ;ˆÛýÂ8?¬í9ŒÙ@
Ööz°@>5_³Cå¿ê)ýêÑðx¿æB]ÌJ,/¿àF–½Š¿éÎÁb‹eAGNbcu?ê
PåRÝÝ?ތî.?£ÿ¡2n'?¢_Ûw÷?ÂÊÔè?Â7ÙoòzÛ?æô‡&¸ ú?È¡(*ÈS¤?·?'måJ¨?´"DHWÉâ?ȎO®*ÖÂ?Ä&ß>ÛÑ?ê¾{œ@Ó?©8Âl:,Ò?ª€ô ç4¼?"'{âÒ?#?¼Ë¨Ï*_?¥‡!Oà?é+•Ói;[?±Z&ÊQՊ?©Ðêpñ–Ç?ž«§Aê(l?ÄÝn¬á?¯0Â^ÆÌ3FGL J0929.4+5013@dõߨq¤@F¹!¬ˆŠÀ9.$I‹dMÀ;7p¯•"?¿káÝL™-@ñxŠ|E@Pàc, ¿ãI&¢ßœ¿ä㹺e/ô¿ãþ 2K<û¿Í½dqfAGNbll?ï÷ä¼~-t?Kä"= ¥?#ø†‡ø¨?!7ÀÙ¬X?Knìe…6b?IµÔ.{Tß?ïËx²å³5?xKõž9Áx?iëÀxÚ?kúæX<Ä?j›Œ¡r¼¦?pR8;˜%?ïtf¼ï]'?€s¼…/ï?u4''W<?n9|rÑ?ˆL<ûð6?zËoõ=Ÿ?ïªmUbU?€*»×}?A™"Ö?H#mÖ8Š¬?"T)Ù?€O‡It'3FGL J0930.0+4951@e§€w‰¤@FÐ<aNÏÀ:h÷´×ãÀ; õ§·iŽ?çê¾±kž@ðÜ¡›?÷&€®ç	¿ÔâªÂêSy?ï…Þ7¿å²6ĕÏ=?Ý\–æ®A¿AGNbll?î÷3)Œ¢`?¡ ó"ÿžú?\íÀß4?ƒ¡cž^?˜k$ED…? –ŸÂë4?ïÅ3vϽã?{Üh]óàÎ?n Û½ßÒ??qǵ3Ñ8?l«­rbKÛ?p"lÂCP³?í:°êåB÷?¢ûÙ¿#¨?©}øka]t?œy8€Î?¢ÖøæJs?"™2‡&%?ï##éµ$L?¤¬¤Ë¢ªç?'gÈxlä¯?£:—é:L5?"gt¡Ý#?
‰˜TV3FGL J0930.2+8612@_'‡aˆ±@=ƒ¬ßÇ{TÀ8õ̏+\À;¥÷´#ì?äCÄeþ•$@,1â%O@xF€B²¿ÙúA©\t¿âœ‹ó1e¿å"Lu¿á\b'áÚAGNbll?ïõD¨pÌs?R…$!´?B?Bàd–ã?=¡µÂ—A‹?H®\i¡ª?LfIíÿH?ïŸrì£	?'ò'¿ñãé?vŸ
Ê»Â?s¡‰ïí|?y§~ãûº@?{É̦)óÖ?îõ©¬'•÷?'".Æ'?‹›Ia³'?"쉝Ïu,?"}%áügC?†à¦f€áü?îÝ	R	†'?›O:äB?6˸#µ?{ÏC•ÙÏ?›Ý:Xóð?™é\ 8ÖÈ3FGL J0930.9-1904@o^à?pX@6÷Û ¥&–À:‡âÀT†À;ȋfÐïq?ñuõjzÈ@
>ä'åp2?ý—sŸ4
N?ï‡HvÞ¦?ïj#hÿŒ¬¿ÙÞÏuÀîÀ¿é"KaiýPSRPSR?í3D·M‰?·ªÑ¥N2š?§Ñ¤Wd@'?«o'c'õk?¤ú}&æÓ?°1‰œ[è?ØåÎðú?ÓvV.Vô?áas֝gÝ?Ó=2À5,?±](÷PÙ?±êÈðúg?èØÉ®ŽÀ?¶ŠK!u?¾:ÿ€!ï?¬'±ùÚ¶¤?»Ê¡h
?¬rm^u	¿?ÒY Ô¨0'?ƚí†*\]?æ–=¢?ÈÄoÁs–?™Ê¿óõC§?¡†ìrx23FGL J0934.1+3933@fÝ]¿Î·‰@GÅ)ßÍZ'À:&æQÙ¨À;õ¯}0­G?ê·ûקFU@Žµ‹è@8RÝk¿Ý¥ø³ÁŸ-¿á¢¹䏿ãhśwŒ¡¿ìÿÊKÏGAGNbll?är8(?Ê-SUsk?֊OâI ?ÉÊêøþàî?•ÉS"ju?•¡]-¡?èœã›šì?Àœ­:'?ÇôÛÏñ[?¾z¤Hhÿ»?¦^W
Iz?£²~#¡øF?èSµhÖÉ?±Û©{D?ÅrГM?¬œ
­÷UÒ?²a.|¯‰?›$7º=Š'?æM'§cX?´™Ôô¬¼?Ï£Ï.¡ßË?²|‰¹s.?¬—±{KU?¢Nƒ Ó±V3FGL J0939.2-1732@oe'@š$@9v·¿õMõÀ9Ÿlr"À;§þ#†íÅ?ëÉï"Å@ß@V‡7Â9 @(Nß·
C¿àÎ1ÏX¿ãmt‡¼Lw¿áöE"㟿íËaè¨KAGNbcu?ï|G&ʏo?‡*[óMÈ?Œ¢Æ21-=?†e‡wgŒ?a-Àl«Üc?]=k¹
¥q?ï`4<A†??Ž¯$F<åû?"xpÜä?€€¢Ýìƒ?ƒÕÝw-"?†)šé?ìO«E{tõ?¥«èi?³û¾ñùØ?¡oГx®±?£D*d¼ÿ?'@o |Â?îjùò:?P~¢òr?'#àäÁy?‹?Vm&Ù? Í°l®{¶?˜e('
pP3FGL J0939.9-2831@p;vm
J@1Ý!ŸŒø¡À9s£Ô…þ²À;¥7†
¢¿¼gù訏E@…®	Ïã@Åt®¶â¿è_ä°Ëö¿ãe€ûñ†¿äÞn´ò¿ïÿ¤vЎAGNbcu?ïí"0ùâ"?cCÛÄeU?ZW‰g^?`)ñëã0?E@)JW"®?GõwÓMp?ï¯ÐL/Å?…°6í£OL?lå7Ia`j?p…£a(Ls?y¥>ClÂK?€ÅñȄ?îDé…f?™·'¨Klî?¢Xm>͈2?•t'Ue?'²"BÍ?"¡›C'‹?ï'èj&v?"%¬V
å!?^æ,՛Â?d"ê†4ÊÄ?‡ßÑÛ®£?'-5çKù3FGL J0940.7-6102@qGÿÞrÀW MRnÀ9ƒúNw\À;]¯"­¡Ž?ïÄ*×]ä@~ëÑL@^d¿9a¿Ód5Ë$<\¿ãÔ/5]ì¿ê"'ƒöo¿êb-à@¥•AGNbcu?Ðܝžh;?Æ´ƒºì
²?äÿú¤SåØ?Éw'ƺð?´´c¿äÌ?°¼s=uâé?Òr¥°¸§I?ÌIq‰¹ ?ÊМùÔû?À0&~|F?à†"e7?È»¿@A?äÜqϳÃ?´|F×è§?ÍÂgÜyJ
?²
ɤÑ?½—¨ÍÙ?žvÖ@ƒy?๱~‡?²gç<¼ð??Ñ·U•Êòà?¶ôDÂp‰?Ì>noýü?°CÞà÷=3FGL J0940.9-1337@okÿÚ@@<g®¿›‹âÀ9«Væ—À;±gž?ÙыÇ㝸@V¹"
ä`@EÜѹ¿áÙú£°Úå¿åû¬'œ¿è'º+×Á•¿àf>"z~KAGNfsrq?ïøO}¬Á?Nh½Ö'{?@Y‹§YUŸ?@dʙmOd?<ÐûKEVÁ?F<ØEêŠ.?ïÎ ÊV?xÕð‰ÆG?e¿·Ã€9H?h½ã'ÓÙ%?l@('µo¼?qN—@Ká?îü±/5?˜LG¬;‡?'¦¥ÅŽ›±?|kÞÀ,O?—‡6–q"?‹ã}Ž'?ïæ€.JR?kW¿FI1?#í"i¸ý?)½à"'>	?hOBݜ–?kpR4ÚM3FGL J0941.6+2727@i$(?NÊh@H
÷Ÿß-øÀ:!>ºOò‡À;øgÕÒ/¿ëŠÝœ±Y²@
í1™*^@õíHû¿æzv×ÞßÛ¿æÆ(»,‰¿å'¬í€Ã׿çÔ`hå5"AGNfsrq?ïÉÃlž?€Õå°ºn?`ä>‡äj?cØ_Ê4N?r¬S¯×|*?||{Riõ?ï{ú	ǘ?'¨>Ù|…?åýՖ†N?‹¬Ïfö¹?~6ÿqO'˜?'4&çD—?îU¾ ~?";2·­Ïˆ?"ŬdúV?'I^EiY?¢Y³)
ä?–£ Œe?ïA%È?ŒÞ?L½×".Û?pאJÕdö?r!RûY1?"¥båY
è?Œ-Ã<ƒ}Ð3FGL J0942.1-0756@nnY!…Æ@@(àaÕÀ:D"ÐÜýÀ;×Ê0:Zo?î¢Ðƒ6@ʂٹš@@‡}?pÙ1?ïþª'[c©¿Ø9î'N¿äÍExZ.˿䪀;ú'AGNbll?ïõ·²D?gé%2£ß?Gÿõ—"W?[e'Ô}è?Aù,+ot?`íc6•¥?ï­ªä‹?eo˜ŒU?s±hôw´?tœöÁO?uyߤÅþJ?w«û!MnÍ?î|ªUD}?™EÂ8"[?˜QØÚu?¦éñžR?˜Tco'¬?'8±_ß?ïJ=Ö¸h"?'è§U
Ò?|Þ·~+±?wT›3îÏ?.ƒ&Ő?ßz\š"z3FGL J0945.9+5756@c"`RP/@F¶¬@eJÝÀ9§#Pg ¡À;þEE"n¿ã3ÿ‹æÔ@–K Kz@£	ÛØ¿å_Ð˒˜§¿á·ڌÿ俋8áP›¿ç>eðŽŒºAGNbll?ïÞƶ5Î
?t1[º?b¹R HÄ?i>ÂrŽ?]vð#[Ÿ?eÓÛÿEã?ï™ÿBEv\?"%côª×?y™X¦+ÞT?vb"'¼@?yg7ó§?{,w[g›?ïOr=L±ã?'¦§dÂÅ?€l•7?tÕ;Ñ­_ê?‹·p«Îñ‰?zA¬nßc?ï‹£~óc?‰;Ã<ʵP?g²çýL'?mêð`œJ?‡QP¦CÔF?‡Lž¸¢¯û3FGL J0946.2+0103@mlÀ
¡©@CHEßÞ!‰À:•Rh' YÀ;¹Ã›Ë£?ã¤aöÑ>@ëréV›B?ûÏ¡‰Å?ïù«±~Æ¿ïþ±²{N?ïñ´Ï;MD?Ä ¾seàAGNbll?ïñÐÁ«±0?`ïu8Ëy?3붲k—?;Cw Ýj?WcŽü¾þ?^údŸJs?ïÇ5ÁD0?¹‰Šö3…?lLG…ä"?xl‡=?l~™¸×A(?q?$Ðq?èû"?'ÈûP8*?ˆ§jú
=Ÿ?{Û塃¥ø?Ÿ5FåÙðš?n¼æ˜?ïz)†{a?«¨–ní3?2{g0Ë%£?["¤Ç–™®?æÍ2mgT?«®?	IÐ3FGL J0946.5+1017@lïàÎ'@Eµ'ÿùJÀ8­@)»»-À;€¿®Y?ó|
‡ÃXZ@	‡±d¼m@©Ç`&[^¿â¸Œ4<"¿çÑëë1M¿è£:µ¼¦¿ç¥ÞvdÙAGNfsrq?ïx%?[¶…™v™;?Q:VÚז?P‰çˆÇ?Qzóœ4ޚ?Saü'¿g?2÷µ?‹144-§-?°4àbî?ƒµª×»AÑ?z
·ßë?zòâ6öÐ?ï&Mæö?ŒšO0 ?…Ï^451¿?m,Æëh?HgBèˆN?'!qOY?îPrþ(!ü?£šéH?•½!ˆÕÈE?'6³kõÐÅ? ?Yü? À*´Cþ%3FGL J0947.1-2542@p.W /µÐ@5¯ãˆÀ9sHÌølÀ;ø˜,²?Ù¯ËàÏ»@$ko9Ê?ÿ30ßEö.¿Óø«oQi¿ß6N.í%¿ÝV=Fåö¿à겆$œÂAGNbcu?ï¹ÎxB`?xáŽ%°?jÊT·Ëž]?hšßѳ¥$?u³™'ê"´?s!}"ø?ïn
EÀ"J?'Qen÷Ú?~ˆçºG—è?wo.],ý?…8ú²Ó¡Ä??¾"/?îÊV®Çà×?ŽÊGƒ?9º-Íæ°?€ ?íæ?—MñÒ?…;¹l-¬ ?í\f(â€?™s)Œ0¾é?…´jÊ~ŽÉ?€…—°ñÈ?²fAf!"?˜{•× µr3FGL J0948.6+4041@fžP >cé@I+ŸÀûÀ9é ªšrÝÀ;ü	Iú¿ü¬iøÂ@ʚ‡«/™@Yÿ¿"S¿çþ€!‰£¾¿çVŒ@낚¿æINa7…¿ïÿñ([AGNfsrq?ïììJ'Ñ?v\ÅyÔ?7ò?[GRe?CtCZϝ?`m…C?u ä=Ø!f?ïµ+¬(ä?'+û6þ½²?rr#^Ó B?uÙ,ÕKJñ?røŒºà0?wãÔRßÆ
?î\2:<?ž'˜"6‰k?˜(ÂýFb>?"9&àa©?œTv»w%?–ÿ5Ês#­?ï¸÷`Ў§?‡OöŒ?T	ZÉíh?e…[´Ö?~øå=g6?7cÿK53FGL J0948.8+0021@m'Þß)@CXßÿ¯x(À7»¯ºmÀ;Y	Ó¾X–@Ü^žà@V©¡#¦£@é‹+홡¿ãøN§;¿é/2°ßäà¿ê"9Æ^•¿ïÿ
1ŸgíAGNNLSY1?ïƧÉÈ?SçwnÅ?|ó°|¥?Eïõj¿?7ØÁÉðxÝ?7µ)½vK¿?ïuµ#(úu?—hTÒS•"?"gL»?"od'àn%?|W;Ò­?ƒQ?Œèw†?ëUË!W¡?«dÅÅb'?À!89ƒû?©AAÖÇR÷?žk'"ì?–;'Ѕw?î‰Â$ãî?«'ºމµ?˜êdºV?¤ªã¼ÖN?•õ´©læ?¡\Š z3FGL J0950.1+4554@e›ú€Ïž8@HÜRÿ" À9ù8¶Ç¨À;Õ
¥uoï?Û´þ,žÍ@‰}dBö?ÿ3˜Ì•¿êøÖçU‡¿ÖT©dÊD¿áf¡³¯õ¿Ï'·ïdAGNbll?ïáÀ"[¡ü?w'(=ü´?[e–~¡ÚS?kXË^Óئ?`e
 ?iç"—®
?ïxÃáÒX?˜2]"Ójp?"&"ɔºœ?" ­âAuD?{dØ{í^Þ?A°ïdœÊ?î÷"é'A%?ŒòZ~gý?‰äZVTÍ?õ ¯½ä?" ¬°ò?ƒœ›ÉC?ï+@&§U?'ê¨J͚?}/ǂkx?€–^çßüQ?•®¦SÏ?ý{j´6v3FGL J0953.0-0839@nř'ÿ@@óàVÀ8H.Z†^SÀ:ÙFóÚWÐ?ñ|Çô ÑF@Úú7äž?üâÝø]Ê¿ÊQʑÍâ¿Õ»ÙÂK¿ÞŽcMµÉ¿ÖtËí¿ÈAGNbll?ïíb"¢"?c»~+#A?D¨+oäÃ?J›!À—P?Zç¦Èv'?]wº¥ƒ'Þ?ïÁ§lJ?{_^+ò?lþž~‹§Y?n°íþ®ˆ?p­-Š•"Q?rٍÉìòÐ?í¢½ƒ??¢t
È#¦©?š5±=ü?'±;'ó´t?¨Ä¢0?;!Ž˜a·?íŠ]ìžÚq?¡Õnc|š¾?xœ!a1e?}¤*5?²#N"ör?¡(Œ‡E½'3FGL J0953.1-7657c@rV@ €À1‡@zC"À9ï›Á''À;ü#Òm ¿à͙—Úìd@ÛXè#•[?þ—‡€½Tµ?î"NX&C¿ÊüýRaÞ¿ØaiTµík¿â¯š
hõÉAGNbcu ?ï­ÈaÊU$?ˆD»Á$?U/ðwÇi0?`s-ÆãiC?çé~qÉÒ?…Jñ7¿á?ïkâoU•<?—οÊ»è?pï"wa™~?ugØo'­·?Œ™îéäw?•p´Äɋz?îešü[¸k?'GP䍾?n€1?}ö–e²U?¡W™8n4?‹Ã¤ó?촙nÙÙ§?§."Flqx?y²ŽêæT?z$_¦öÃÃ?¸À©"n?¦DŽpùi3FGL J0954.2+4913@dôªà~Zy@HÉö`D
vÀ:©î,˜å?À;Ë¢1Ð?äL´Ø©Í@°†'¡Ú†?õM9§š¹?îwÂ%Ì:¿ã¤ähŸÑ—¿ïÂ0œÞ{)?ﰋ֍jâAGNbll?ïH¤Iv½{?­ƒ½˜@©?q>{"?"ž<ºû?'›Ø
‡L>?¬rÝ#Ø:?ïºã3-¯?[Šv…ûk?rÒ²$'§?"¬`žqQ?owhš¦-Ë?}°ª"/Ǒ?ìy®sèb}?¦À¶ÔO~?±}Nš_/?£_6,?¥iþ$EÙ?•ªpÌùd?ïZO¥»D? mk~d²?f`KÒ¨?†hÑ爲ï?'êâS—?ž·k¬—>$3FGL J0955.4+6940@a®+ÀãŠ~@DE…`&±EÀ9A¢e6À;Ï"כ\è?Ñ9Ô
x@
xjRWù@®#ÿ¹‰#¿ßßëÄ¿ÞTžç·4¿çÑ,ÎDœ¿ÛÄę!¥OTHERsbg?î+u¼¥à"?°ºîƒåÎ?ªÂ€µK¶®?°$ì¹[?t1²?|û;>é5?îLÑà?²¼ùiÀ¹v?¥'gr¢ås?¯š1A÷–?†³-ï|e5?–û"(«F?ìSBVPcV?£ß+ICK?¯Éؽ;è?›¹é±{¡œ?«·Â<Ž³?–Fœ+µ¬o?êvûýMP¾?¹Úü*î†Î?»Û¬hv?¶ìÉÜK ?±,9éœ?¨ðÚ=\E–3FGL J0955.6-6148@q»-ÿ'+¿ÀÈÙà0¬ÆÀ9…¦ a4À;dM\‰?êÄG©³@
}~
@›_¿®+L¿å÷ó4Ѫ¿â·K:Þ¿ÛY6ÿ⺿îÏ
L½¦rPSRpsr?ÌÔäü3M?Ãþâ`¢Yó?Ö¬L(ݝe?Èö}¼Å›ì?ÚéAYÈó?Ê@á˜ù0^?¸''ŒÕÕô?»rJá¢'?Ö¶%ØÚ?ÄØ?<¨qŽ?áßònÒXÕ?Æò½…Ô­?ä £˜1I?³}ˆèÖȀ?Çý@ÆÅh*?«ÏÜӟD?ŀ0ØÙÒ°?ª‹2ڟÍ?áCêì
ù?·	äì?Ç}?£ò,!?¶‰'p4DQ?ѹŒ,.Íþ?³ÓWŸj•3FGL J0956.6+2515@i¯?p]@Iwù jn3À9!Áû¸r£À;²#ÃS§G?ðÐój›TZ@ÒPw¹Ë@|G '¨;¿ãGXÕ6Ü>¿äãëSdoÛ¿è_EüŸ´w¿ïÿ˜µÁ²AGNfsrq@?ïá8?íùç?sB_X½ný?h;M^h®?qVTçʗ?J1ÊÎu«à?O~܍֤t?ï{†¸Œ?ršG'
?'"qЂŸ´?…»wՀ׼?}uYêûŒ?uᑣÊ
?íìŸÃ
iõ?›ÉP"x¤Â?¦"éÞGÐ&?–C"mØ?•b3â# ö?ˆî"Èv?îљÙpñÔ?˜ìýl²ì?•2u"¶{?"¸X®†Ø¢?Ì'\]Ä?A½‰»O3FGL J0956.7-6441@qك @ÀÀ'{ 4hgÀ9´Ïú~¶¿À;}hq¡›¿Ó>ehIÀ@wZ!‰'@Ià [R¿å•‹g>§¿é‹åô¿å	=Éí¨¿Ó=X™&àAGNbcu?ï™7ª§?"ÍyÚǸº?_ŸÔM"Ë?aƒC}Wõp?Œ%·‹ÇÕÒ?"-M¬…á??îrÁNn?­ˆ"U\QÍ?tœ"åÑÒD?|ÏÏi?¦Ktw0ÞÎ?ª—h‹5üµ?î\¾f;#?•GÄÄW±?'	$\áþÙ?}+tÀ–ý'?¥Õ¡ë+NX?'.@ÁU€?î©ß^»G…?"ë²3™R?F qÍs?K•åâF;?¥‰¶"S3?"á±e»Œ3FGL J0957.4+4728@eA¿p@IIí )k3À:¨(÷À<ÿ™¨³?åðQòċ¾@"y$én@[œ@gú¿Ùftlþ¿éÅÿýËÑ¿ïj'"?ÐÅ@CŠµAGNfsrq?ïõ¿‡?ý©?xtPÉõÿ?L;>Ù\yn?feýèé,ÿ?9HMYÎU?k£ºÞU¿?ï©&yáQ?"	hsu?yHª@û?Z)¾bµØ?r$®˜Î]?|Þ!_ý?î\†€ð8 ?=lT®¿Ú?Ÿƒ
ÅÁ.,?™ÁWJ"?"ì%7Í­?ˆ"«É{ñ?ï¡jØ]ÔP?#"~H&'?jŸXdì?ÓÂù4??€ýsχ°¾?‹•x'Ï3FGL J0957.5-1351@os Æ´…@?.²˜¬4À9_ÄM¢JBÀ;ªFX©åA?öfàý0lÚ@wŸäŒ\@)=³ê¨«¿ás؉ÚP¿æY<Ž&¿ë8ÙP;y¿ïÿ"û&ýEAGNfsrq?ï骘;Þ®?c›®Xy?bAäc¬?b>\H\Ʊ?A—~öœD?=ÿ°ZlÏ?ï–òÁ¥b¤?‡ï˧7ž?yöí"Ó£?zí¹'•Ç\?zœ?ÉÚÿ?€Úk#.¥?ìĵ{<³?£Hî/3€Q?²ƒCV.0×? wQ"m?\CC_¦]?'z›Àn¦?îìÌÆ©ßg?š8[],ðæ?"‹"³?"6 +H*^?Ž§¸!ûÂ?­¼Ü'ÛÕ3FGL J0957.6+5523@cÒó@ÔÜf@GöãàÈñÀ7nû`^À: u'ÊI?øÂjž.@
ûãL@€?ýÌðW@"¿ÙNKÏié¿àšÈ0ŽpÏ¿àÕ£Ñçúâ¿âd»rv-óAGNfsrq?Óí´'Ôë?Å'`þ¨Ï?Ñ@¹Æ˜˜‹?Å©˜\†K?Úђ8?'‹?É[ÍU^ò?ºÑ˜'̐q?DZ®ë©2'?êŸçw¹ä?ËéžÃÜÇ?°6Xœu z?¶¼±X•¬³?ß6-:öLÙ?²¬\¾›ÿ?È"Ƹ}¦?¬‹•Ì"?Ô¸ohÊà%?±ñÅ婸§?ªCØà7BÄ?¢‹å'±5w?äWƸŠÄ?ï–,A?Ô¬ÕVˆ!?Á••&× +3FGL J0958.3-0318@nD¸€®@C.^è¬À:uÓ|ê6jÀ;—ÛBö?ç±Ä‹_Å
@
wã'_c?ø=ÖÀ¯?¿éśžæ¿´Á¨Æ!%Ù?Õ<OÞÜç?º¹U2AGNbll?ïö'<Û?NËÞð
€?BM)"øø?AÝ­%7¦?C®Ð"¢à?Eß6N—ئ?ïÇôÀBU ?|*º|›¶?jS!ç?pmRKŠZÎ?n;jˆøÅ?qàG¢/ã?ï1¸t"Á?Œ'¯é±?‰º2KJ?héaxÅT?'jk¢ÔBA?'äìr±M?ïˆÊù`?'T›nàž?=õÍt˜¢¢?Z¯Òºm?ŒÝ"<T[?'=L_3FGL J0958.4-6752@qû™€o&)À$Š>ž¡@WÀ9ûͅYqÀ; ô‰u?Й¼(ÃK@
áJòA¦i@§ø`ygu¿ëK"ÞK¥E¿à`–!ƒÍ¿ØP¿ˆõ?¿ãf"Ú ¨ŠAGNbcu?îl#´-é6?¬Šž¦f?hŒo^5}T?l(žA…iÒ?§´ýÇ>Ó?«nQڃPï?ëÃ9sO8?½©V?Ó-u?"R­}é?˜N²îÖØ­?¼Ñ"Á¦Ç?¹Óüi—Ά?íÝÔé(?›¥dyeÛ?"‰ÑÉo¹?ƒbapÈ¢‰?§Þ"'vv?•ñØ÷òV#?íÄU¯É…\?šI7"Îhé?xtäq¦"?u¶Ø9†÷F?°V:¢:¶?˜ÖõËä)r3FGL J0958.6+6534@b82€ñ,(@E&Ÿ¦ùÔÀ8¾­µ°P•À;ÁUÊ6ðW¿øv†PÀb@ÃÖDDÓo@
@?‹0J¿ã•Ó€ná¿åÒÙõ‡à¿ä-Í÷!é¿æ®ƒZµO¥AGNbll?ïúägÆPê?=²|q³Š?ŽL4Åm?Õàã"æ?A<=5¾û?<~?°"×?ïÖ7®'…#?w]7¤]?a'N{ÄÉ?i.UGTðµ?h6A‰ÿØ?o.¨TE?ïk_ûá<?€"s1óý±?sB(¬«?mdn±ùô?‹†ì÷¾Z'?{¨S_Šõ/?ï÷ÄFÀ£?V•RP|>åݬ?Ž»"ûaY?PM]Öėù?V{¶0gåƒ3FGL J0958.6-2447@pDêŽ:Á@7pæàtI~À:
ZÜÅhTÀ;Âá½Ùà?·3Q7Ágˆ@XÓÞå@ðp¿…¼m¿á\ï»Ü¿åºH싌™¿æ\wÜtNu¿ÔnRÍF3AGNbcu?ïŸ[œT?À¥>4öu?qÆ*¿*n?{\©PÓêú?~Œ«>̛?…¢ü€{ø2?e,X?ŠÉéðNìK?tïþ
B]?xžpvh}?|2Ï2'wß?'«l‰_e?Râ|O?"Þ>¼U?Œ©Ïî»?€ÔŠµÆ‰+?š6í¬®c?ŠæPÍÂj"?îþCâ¤ý?'Žk‡$Œ?j\ðG?nL{¨w&ê?œë墚?' Ò•Êž3FGL J0959.7+2124@jtþKZ@IQ4 ½À:[®a§ºÅÀ;äEÞ0¢_¿þ‡†AM'P@Þä‡(¨Á@) CVí?Õ®ï1%¼Ó¿ß"ç†óŠã¿ë>ãp?›+á
ÈAGNbll?ïÌþ;sš‰?…³î²?w–o/€?…4žxç—?C'a6`‡?G‰Áúƒv?ïÑ6çËÀ?ƒ/`g[a¸?hlŸ"JË?€"U­xBÅ?f]Sþ óƒ?kt‹K<â(?íáJ¸jÐ?¡ÉÂnÂ?§ç¯S«_Ù? Mè@ö?"JKeæO?'òi™&?ïíÅÄÌa?eúäT´£>õÎg®É
?ߌ9;ϛ?b·kÖg?eù·ž&3FGL J1001.0+2913@hî^ß)@JK8_ÂÞ7À9'Ö!à$˜À;ÁCÂÍoŠ¿ô‡XC¸çh@ï1Æ̂¥@A›Ÿ®0ª¿á;™Užd¿æ›Siñ¿áhòüGŸã¿Ó—Ãl7AGNbll?ïý=*ù'L?3žê-â¤?²×GBjÔ>ÿ½Ð^j|?3€MKSô?2õ ÂR`‰?ïԜA£{©?€(ÖXþŒe?f46~|[?zŸ®Fzo?e/‡Þü4?lŸd.îér?¥J«?~¾RÚf8?p'jwºøH?iÆQnmŸÌ?†QaqwÀq?z	^žô]?ïüús/Û?>'ûc'Ù>¦±¢™@èE>µfSv«?8!U4°?>Œ–¥o¶]3FGL J1002.3+2220@jPå`A‰7@I¿f€g™lÀ:d~¡ÆÀ;à\d"ä׿ǃ'Ù6Ã@ëþ<[{@x¬ßœˆ6¿Ý]ޞl£S¿ê8Šò¿Õ2–È%j•¿èB`é"]AGNbll?ïÖL=à¢w?xØA"Kv?Y፼4?a¦3œ£å7?lÂûšÿn?u Y$¢Ô?îÉp¿7q§?¤*3"mL
?˜Õʍ>à@? èé™îô—?‹ø;¥ÕÃ?ŽûۊWâ?íÍ"$92?˜à΂Ý/ ?–¯ ßl¥ë?‰jTk<Ž?§Ö
L·ÙÐ?"{ª 9Ïf?ížü¥È9?¡®ñIÛ¿?‰}Æó1'°?†ôˆԁ?¯°Ãæ±ò•?Ÿžj5rB3FGL J1003.6+2608@i"&?šIÃ@JV<ã.À:nˆö´&äÀ;ãØ$ãý¿áYZŽ/ÇÞ@
ÃNÿl‡=@UÎ 3ý¿äÜ4~]z¿èñ*,××ö¿Ò'i!à-¿êŒ²$ÒÏAGNbcu?ïyË5õ'þ?'½ûª­?k™SåòYS?p¶·›eˆj?Š¦Ý‰éú?Žµ†32Ã?ïwy³è†w?#" Œ?ƒv林Œ^?‰ež-0
?}UF¼Sª»?žu:–¨Œ?í£aëÃ'Ä?Œw"(£?ž`Kv-W?'4'	¬{?¦™»ˆ·?"4Fl{©9?ïä^)7š?Žlˆ3‡»?c?¿Ì¨%<?dÊК­î?š[|AD(?Œ¹j{4¡3FGL J1005.0-4959@qYBà°«@
Ý¿ä1À9 –6—À;W¢Õ'}ô¿í¾¾Ë='Â@
çEgée@78¿å׿é殚T!¿èrWý(E€¿ç.ϧ%Pû¿ä"0™[ AGNbcu	?íás\ÁéN?²5"Œž•J?†K¯›'sa?‹â^6AÄî?¬UÞMÎ>?°£ó#-n?ê¦Í¹s{?ÄÿD"'¨?‹@TK+YN?–$jˆš?ðÃՁ0€?ûŽ"þ±9?ëPŠ)'&?¨*.ˆã?¢Ž¡Ùæ¯S?ŒÍTUÍ
ù?¼4]Êà%?¤ÌñÛp?íyB½Î:e? Rƒ"A?aöÁ'?aiµ`ãÍ?³¦9¹ Ã? 4ÈæÁd3FGL J1006.7+3453@g€Àð¸@K6îÍ©À:¾ž\vù\À;êň4íH¿×ך3{
@@
cJØkf€?ú|R@¿Ê¿ïÿ
ç\›?ïÍ"Ê5¿ÔÄ@ٱ뿹ܦ/eY‡AGNbll?ïüzÚfã‡?4Ás+…Õþ?-j@!åqR?,àÞ(Ùú?*èoâ2—?&‹"^†"?ïµ\kî?"œl^¬?tW lŠ?~ê•fJDY?qqú¸hŽJ?tÊZ'Ôl?ïZ›†
ré?}ŒŽtyzU?€È>ÕÓV?sŒÄŒãéÜ?ˆß¦Ð0]?qÊ)ɺ?ï¯n³yÓm?ƒ‹2œ?p¿'÷KE?sÃî~ÏEß?w‰#KËC?ã%6臄3FGL J1006.7-2159@p<۟˜·@:ȖÀ¡E`À8¹æè¹À;ŒÕÓËò?Åò´âd'Œ@.ÁКaÁ@z›@7Ӂ¿âJ°7S¿çæ `U¿è%=ÍÒŸ¿×Æ*g˜Ñ¯AGNfsrq?ïós`ÖnÓ?U6û<ðú™?DdÍòKÐÎ?C"~ŠŠn0?MÍ®³øå™?Pƒçe®}½?ïÈÎ+ °?y샷0"?f`ÄÇè;?f穛Tå©?phš¢4Æ?sðr™
—­?ï?~gîZ¬?‡Žd¯Ÿ?z¹aý؎|?s(Žõ²®?'aڂ¾†Ú?ƒîwlþ…?'ï9?Œ"±Õl?IL´4D?P¦@ÚF'?Œ
xð>¢?ŒDVÖ¾â3FGL J1007.4-3334@p¾%`A‰7@1é¬ "ÚÆÀ:Ž(LOdÀ;¥¹¯¹–?ñÃv¤÷ñ"@·T?@N[ÿ…0׿ßúú¾]Úb¿èÕìÅTw¿èq…­Ғ¿ïÿ8Ýl,NAGNfsrq?ë$ÿã3%?ÁMÞG7HÕ?½:`^ˋ,?¿C0g
aÃ?£;A7×S?©
b%îÐ?å0ð?È=&ZsN?ÐMV¢Ž?Ãü>ÌåǗ?µC%SA?´Yßå—Î{?æÆw˜Z¤?µ÷³dŽã?ȆÎYÄs«?±0]J¸ç??¸¾«?´CŽ?¢¤wbiû€?Û#Z^l?»_a‡Nvì?Ü[âD6$?À2"ñå{?Á,0Þúñ?«û7½Ê!p3FGL J1007.8+0026@n?@OÂ@EFv¹ÃÀ:BôˆÓx¸À;Î))Äõh?×Íí"äg@²A±%@¶'¿t?ïýÙý¡¿å"­·]Ï¿¿×®O½Ç:+¿ç`n©š²bAGNbcu?ïàk% x?uÅ[
65÷?Snæí*D…?W~¹½Œ¿?eÝgiWeÂ?só£…{²?í+Ly"‹?´ì«.Mê?°)f2É[?±º ËDµ*?™ðØi3Â?›r+°¨a+?î½÷ɳê$?Œ…¢n¨?Œ59
="ˆ?|uÊâÌ*Æ?š&jBãñH?"Ù<ÒÇì?é$;ËÊÌ?¶\œµØ¼L?µ±äYM?«½¢ÜHb?À–ÂÈ#1?°üïÍ<Ïû3FGL J1007.9+0621@m00ÿì·@Fÿì@/šøÀ8õ¬Á"ŠfÀ;}X¶zzð?ï½ÅÀ6@Aé;îB¾@@<`ƒxp¿ÚIÿ6Ô¿å9=–ìô"¿åÈ,Ì礿¿ág"j´AGNbll?ïÐË©6B?tD²)«1B?jý'mdÓ%?mÄZ³¾UÆ?d7Oédëd?ci™	R/?ïYBת?"ïûT"7®?ŠöSH†?Ò®Ç¼—ñ?Sm랬?',ëjtŒ?qx­>?"QöñbUÌ?'Ñ®Àu‡?…>¬ëF¸?š")âÂ?6¹acT?ì¢PÒ_lü?ªÌ&•Ø¼Ò?£ËûÄє ?©G1ö?±{Š›ÍÕ?§ê.B‹ÃO3FGL J1008.9-2910@p"íà
q@5cÿƒÙ>À:.'Gl¦À;ÄÁE°
y¿×ÑkJ¯Y@ÓÆØA/@ à"ªÇ¿ìD]|i¿ãèPÔXÝ<¿Ñ»:X–o¿ìànà]xVAGNbcu?ïI[Þ+‡?žVxÐÝ	?ˆì"ËCï?Ó<?1?"¬ƒ©Ú‹?–'¹L€à‹?ïn¾&Õêö?ÈHdàM?óðÊð?~(rªŠ^?ƒJuV"wF?…ÜÞïê¼?ìÎCÒb.?¢Ö+Åñ‡e?«ÉŸédÿ²?š ³ÓÉ)º?§R/ùtÝ|?•Ä{ß	÷$?îõ|œ˜<?ÐøžÛ·?i>aª¾Â?lŒýí":?žv@7 º?ùM 6»k3FGL J1009.0-3137@p®…×E@3¥Ð]óÑÀ9¾~ÝU±À;jõ2F¤)¿ò\ªÈÀù…@BN¨Ú@ÈŸ~µé¿Ë×íÇïz¿èn[ø¿ã=;þ¿àáH2¯æÉAGNbcu?ïpÇ/š?Q]Ë\D?Œ‹l,Ð^œ?•,Åú?L1¶]›?"òyKMXi?ï‡OaªïØ?'ȃŠôó?t‰W'É)˜?y"É´Í?ƒç{Óßu?¡Q,CÛ3?ì…IG
ƒ?¢¼QjžR??¢Môt•?'Ý{Iq?²¯,M'-C?ž4AQ–âP?í&'kë?£îøØ«?Z†ô–̵ª?ZªáŽiÑÌ?¶aXÔô-Ð?£Èª"¼4a3FGL J1010.2-3120@p®Ñ`4P@4
Z?çvœÀ9˜
¨_/À;"30®ô¿Íš ;@ÔΎmìm?ù8}_|<g¿ï–`p?ØÝ|v·Ü¿±ëSBÃ#¿Ð9o•í›AGNbll?ïý"Ϧø?<
÷`>ÜZ?Ö`GŠÜ?(ÿw͜•?.ÍmŽ
˞?9Ï¿"?ïӼ̏æó?yS4æ¨}?`QÏZü­?cüþÛ
?kÃá ¾h?sÄ:FÉö?î(áPø¿‡?ŸÏÁÛ|Î:?•goî.?"fñ(úT–?¢¾2ù\ùÂ?™" Àb=d?ï²ewïÎ?'xþÕsd?åïóÀž~?""¬!:á?ƒ<Ö$$þ%?'aô‡¸!M3FGL J1010.8-0158@nl»À n @DÏPßìdBÀ:+î^íÌ!À;ÓN+>?ÀU¤)ó÷è@⧊Hò@	4¿zSÙ¿ãè(b}V¿æ!\?µ¼T¿ävÌsP¿è4í™1PAGNfsrq?ïóÈéR$Z?T¡%¸rg?9ié
rc?4%r8©ÃÑ?R³ZÊ@?Qþ¤Ô>e?ïªQUÞ¸?€*ù{f
²?u¢ò!ü…?röŽx0¡Û?u4cV"?v+У"†…?ï"KOT˜?{ņâ¬?r,Ñ2…í?b'K?²å?…åē'—r?w™ø2Û/?ïN÷`úÉ?‡bÁþF?oÙ±è3h¢?eäü	aI?'%Ý£ q‹?†»b)z&3FGL J1012.0-4235@q#,ÿ§ël@&kþ>^à`À9ž9Pƒ¦À;…§ÉÞ?ôŸ^<vRî@
9""Ï°W@9nà2…8¿íytí<Ú?Üÿ<ÊûU:¿á~ˆ²S[¿î
Š°Ù¸TPSRpsr?Ÿ\`Cß?Ÿî<à‰GF?í|}°?µà•J ×Þ?¯Ú7÷ìU|?²VA:Û^þ?—Q® ‰3`?¬¤¢y—¿?썜T\Ç@?½Ä¿bUp?µ¾±´÷y%?¸ÓÜ;‡B?Ñz¼ªHu?±`X%¢ãå?âƒ{yÌ>?´h.ÏÙ?Âü˜Ä>u?§[_ñ~?´_€ŸNpY?«ßO\ôê®?ì€Çýs^?±Ë²|G-?žhýÔc'ð?˜«jà3FGL J1012.2+0631@mE:Kâ@G?µ!µÀ9¥"÷si"À;"ÿ·¿ÔGpõê @ +Dý5@›{Q^—¿åρZ]™Ž¿ãþ À'¿â©W'Á–Á¿Ô@ßu"AGNbll?ïäšÒùÞË?p™}5èSS?CL,Z©ø4?=ìÚ^$}?f'!ïvµæ?oÓ,€.?ïÃKz4?xí5ú³"?n'*ÇSó?n%˜bó?næÉ¾y­?pÎQ-ÆH?ïQ;'"?'Yz¬>Km?|ƒŽ´ãŠÁ?q B™É,Ÿ?z©Äév?zIö8H–¼?ïvcÎùÒ?ƒoóÖ?Ez­½¨ß…?HaPš#'Ä?‡Ê83~Æ?'ÃüÊÛ/³3FGL J1012.6+2439@iøn «†@K+|à%o%À8=†Ñ™»À;S=Êeê@?÷¨¤&æI@WƒsèZ@ïJݤ¿Þ;:žaw¿ä.ŸJç¿åؼUl¿ìК›»÷AGNfsrq?ï†Ôšé$?‰"Áùk'?Š­ç׏‹?ˆ#—1pˆ?\î™q;?Yڛ·(\?ïÎ5îrÐð?|hŽºm–}?h+'SÖ®—?s3@rÁ€Q?iž9Xa_?pZÒôSê?èý7Ýà÷ú?°°zóÏß?ÄådŸ£Qà?¬PSÑz&Ö?¬–ï£c8ê?›¡'þN4Þ?ïçJš*D:?q'W?Ô!`?<MÀVâ?S`øaKÿg?e+­ÕºZú?pF±¤‹3FGL J1012.7+4229@fԀu@K3N?þó'À:r±ÎCÅÀ;¨¬¥åØ7¿âb¡Úà%@]lWA/u?ú‰ ¨+®¿çþ¶lÛ¿ãñðPh+¿ÂOw݇/¿Ó´í¡ÈVAGNbll?ï۔é/Ý?¥•æMõu?9l',°g?t4¬è-oÐ?pžÂUFwŠ?£þ*ÇŸ?ï΁r0[ì?zmWñ&† ?gâR7îÖ?pZÖ}I'`?iœ;˜…%L?p‡ç‡Žâ2?ï‹Ü׍1B?}yƒ¥
&?sƒå(ëµ?m2ë8=?ƒF׈±9Ó?wlˆŸD
ó?ïÆ$a˜,Á?u­õÄÑ{t?/´çvNJ?¸åRª?|·oʲ?u£Ü^ÎÚ3FGL J1013.5+3440@g̸`™Ë@KÃC hÀ´À9Á/¡®;À;ÐsۍZ¿çنO@  ïX=@þ¸ Bj´¿áLã1£¿êt@;%è>¿à
ù¼«'È¿ïûàˆìMFAGNfsrq?ïﯬ?#?lÙ/µ?8ýÂØ`o?>oÁ¬IΟ?Za6iŸ@?l"Ð1pß?ïƒsùÉ?‰}Fà˜Ú ?B%xŸHÃ?}ä'ì'ÿ?/ ŠÕS…?€?`ÒÎk¸?ï"Ž.ë ?ŠgaIW?…ó
c³¬K?y~'¬SEš?´´ðÅu¸?…uA,þ?ï,€.˜Å4?'{k{½?r֎íõ+?v#ËÇðí?•ê"‰+Ü?Ž+u¨ø3FGL J1014.2+4115@f\ÍÓØ@Kwÿ´€¦À:a)ë‹ÔµÀ<‡ð#éê¿ÜÅèéMY@æ?Ns@c¥ÀnoŸ¿¼UÙü5E1¿åìÖÔà!¿âì/a¨¢²¿éKÍ&¯AGNbcu?ï1ß3úþ?­],5?"•ÚŸ'?­
c"ÿ?`z	cæƒP?fÙv="!?ïx?âÛ`|?¹(Úªz?ƒ°Ï{ z?‰~î$ø«?}¢¬óXe?€ì(mt?í²Û·@?œZ{:M ?£ÃD·C°?"_é<:
?¡j{Ûö? á)AÁ?îøH°ÛIt?"–'•Èº?€B)m*?y&hHzb?˜öH؂?'Ú'pj›A3FGL J1015.0+4925@d±?Ýe¡@J[‰€Fâ=À7%cèä÷À:5›Jt?ì"$áûvó@э7`"j?ýU®€0'î¿ÚªðåÁ÷m¿ÚÔm®6è'¿ÜŽHõ¿ÙãÔåŽÔ]AGNbll?ï·jD}P©?"õwjÙs ?Vc¡>(š?b?®F÷¸¢?~²™ þ?ƒ!nԞO™?ï" %"|÷?Œ'=d?}2åà?ƒz–+0)??x½Ý³Û¤?."¸?éÎߜOm_?²XˆòDo? Ši­
?•W… ~4?ÄÄ^ôW?±
o½Þ?迊¡`Nl?³dŽ†¾í?'_‰…W—?"CFÕq?ʵäIÓÓr?³&à\ëN3FGL J1015.2-4512@qC$ÜY2@"ÊÊërªÀ9î"
>À;•¹Ù«¡Àð'äÄeJ@‰ý²rÙf@é4Â='¿áSó:¿à
sÒEí'<|T‡?×ރi½šAGNbcu?îl\ñJ?¯«ÄêK¼÷?Ÿ!fΨԎ?¥°ŽdØ?œñ
"-é}?£ƒŸrD½?î‡@3ï?±Óƒ<"+?e÷'Ž8?pjýsä2³?¦¨í3˜9?±}SóÖö¹?ìÙbÇЪè?¡*¯RQlÏ?¢É¨okÔ?'µÿÛD"z?¯ +ŠM ?™….áLc?ïð2­O<?g´ø0¥fã>»Þ•
dè>áS)6àà?^Ø£ÿä?g´;HmÓ3FGL J1016.0+0513@mb€'،@GƒüõŠÀ8K¯é(À;)€,?çAÎüýÂ
@@–Ì_¿ƒ@õß_÷av¿á°à.m?¿å»WeÜA¤¿Ü÷¹èø¿ãw×èè>÷AGNfsrq?ïü4ç§f?9MtÜ–,?°»Ä~X? àuø¿A?7ìºØ+®³?5j¼›è	?ïÒë½à¬?y#'W§d?e¾ÖtüŽ?pƒ5=?È(?gUlyWO?m®wrë<?ïfLGC"?ƒ.mäqe5?s€'c>‡ ?mUjü½ó?Œ¬è¼×g?€ âä Hv?ïÕO‰êF\?t&­¤ 4?¨ò~JÕ?/xü:ó8L?t嚷ØÕ?tL¼I"¯3FGL J1016.0-0635@o"ddIV@CÂb¿è¸¼À:A/)¹6îÀ;ÐìwŒÿ?é˜O·Î8@6§µ\™@Z]ÿ—¸?ŒóžGÔ*¿æ*[—ö¿íK£'è¿ïÿ°FP¾¬AGNbcu?ïsýóc;*?"qháQ]‹?WÓgšùg?'ëxòà›?]E}ü±àÙ?k‹#fä	?æ2ª¼?ƌ"Š¨?Ð8ZH¤?ą…ÚL+?­xځú¿?¬vÝ«ºãÙ?ìgüº?¤÷ÕðêÿØ?´Ã6ò)?¡c6Èò¿·?¤™¡(z'?""Âۍ7ë?×ì7Ћìß?ÀôsUª²_?á–áùÓއ?ÃћŽÌCÛ?³˜ï1XK?ªÁ½
<‹±3FGL J1016.1+5555@c'7¼]ê@I' ("tÀ9ÿÓ3[AÀ<Š7üÇ?'Ž»Á¢ý@×`Ô+:ì@3Úÿ•võ¿ä>"èÚÊf¿ç>y|1˜˜¿ãW{¥ÎíJ¿ïÿÍ&}±öAGNbcu?ïî>õ,0ó?jäiªí?E·äšUc~?c[u"I²f?X¦#Zsi?ahE@}{t?îá'ؼ™°?Isëk©?—LàTÏ?™uƒ î"T?‰™A7ê;?‡Xã{
F?ïI(ݍå?‡GÍ;ü¥H?ˆ0ˆ"î?'æcwºå?……G)Øl?x¯GyÓçD?îÕHõªâ¯?–õ°wè0?"X){³¾?‹Ó:ò²à?'þ·Îàö9?(}÷VbL3FGL J1016.3-5858@qÁUÿæՍ¿þMV¾|'À7s­uïpÀ9¢ì,
¥?û&…}'âž@¼œ®L9@GÔJDœ½¿á¡—Ú§¬¿àÒ¡'Ïe¿æB°ÊkQ:¿ìU}ÃOJ–PSRPSR??©GBöæ?Fø Š  ?â%esz»Œ?͙Ç:¯‡?Û­JÇFø+?͙ìŒ}?j(º^ǎè?y¤A	´‹µ?äg÷#•Œ?ÇÛw³ßº?ÖûÀDXÌ?ÇÚDZcù¯?—ŒhìæuH?‡öĬ¸ù³?᳒{'É?·#X¸›Ô?Û 8;I?¶á—9ð&?Š™âQP:?‰É݆™›?Ò>jgüú?º¬>ü3Q?æx\dx=¾?¼éÎُҭ3FGL J1018.1+1904@k1  ôØ@Jýb¿è¸¼À9³e·ýäÀ;§'ûç2¿ìŽøjNAE@ؾoçÄu?ÿ¼Á¿}ƒä¿ç2lw*6"¿×ׂÍ2¿ãøãÊ¿²ïæéiÍAGNbll?ïúÞ(#ŽÕ?D*Kºp¢Ç?)ž‰üÀ¨C?*¤'_ ßÓ?<?yå)
?@rù|`r?ïÔ䋲?x̬
Â4?d=°"4?nꬩ떘?fÞsߜë.?lÁi€Òö?ï†i7¤V?€8Á¥"l?{38ÙÈ'x?z¢PóÄ?€ÌªDö?p°LóRù?ïäèûê™?f¤ˆ›—&?™¢_ag?«yØ«Ñ{?kœ°z—áX?f"³ýϓÔ3FGL J1018.3+3542@gŽï€Uûµ@L:. &{•À:,G"GÛÀ;ç¥b$¸F?â³Ôœ±d@äDó¤ýÑ@d'Ÿ¥!b¿åŠº3 žú¿çë}®ùÊ~¿åË©tX¿ïþq|ýAGNfsrq?ïó xùÏ?&D+#CÞ?—éC'?#Âô ¼Ê?XN­ËÄ?%d"Þ?ïr¥Ó"?¼  õêä?"÷ˆB`è?Šlœh)?|¾ì­/3?}Ρ·»D\?ïT¦'üp?…ž˜ýåÞ?")<nDD?|¸ŠZ"L?†GVžÒŸc?~#.Ù¯óí?îË'ó<?™…É'RH?"»½¨ôØ?Ž¥ryßÝ?'â[X£Æ?ÅLþ2*3FGL J1018.4-3119@pÆp_®¼A@5!@ÂgïÀ9€÷¹à`þÀ;ëg†ù?ðzÁDXt‹@¤æÛkÌ@D…ßÓdÁ¿Ú̆žó©8¿èsá".c¿ëT³Ý¬\Ú¿ïôf¶1C´AGNfsrq?ï1Fu×î ?š'òLpÞ?""øƒõFv?–Ó"¡Ì?yã3֐?{DÌyò	i?çH>Ší?À	žN?…?ʇ£A1«v?¹[Õ1"¦?°®É9EA?°\—-=S?ì9ñ®Byp?©¢éU¯mÌ?³?Ó²š7?¢=µÌ7ˆ®?¥á=¶£f‰?—ÌÁ<µØ0?ÝØ-½vN?´˜‹"¯åR?Ú6‡g½•R?¸–b§iÓ<?¿Å.Jш?­ýcZ½‡3FGL J1018.5+0530@m–/IŒ;@GÙUÿæՍÀ9V‰µöÇrÀ;S 'àð?ñêâצ°@l"6Ûß@ΓÏ,?îMKMV9¿ã ó粛¿èk¡—ÐýÅ¿ä}å-AGNfsrq?èšA®÷½?îœmû¢õ?ËývÝ QÉ?Ãwê>tŸã?‰˜&p v?‰"bV_ò?íÔèNZóà?·hJ¼ó	ë?©¸ÝÖD|¾?µ^—›E¯?'ñ:ˆŠ?–HËÏ­âÜ?ê'óP0͵?®üïÆßx+?ºôt©J•j?§Ak&o?°sðÕ.üð?›ü¶ŠUY_?àßÅFoÌ?Á'Ŧ…}á?ÓǕ]v?Çíc€$?ÆDÄS»…å?¼o¬^…3FGL J1018.8+5913@bî´ßݵ@HJa€M˜9À:ilØ{À<&¿è+οñ~:Ãu`@ȈD‡™@¹,?Î÷õ¿å›Z—ŽI¿âYl"=·¿Þ^…Ø'Ê¿Øó†FÍç!AGNbll?ï÷LÊîÈý?X¥ÄðÕ²w?Euô²{,?U±Ü‹3FK?:­¿$Á?8z]Íù?ïȹŒjl³?'Z‹±ñU?kå¯^ ?~ÏDÞh?kaYæ5F¤?m7P
sÃw?ïO4NÅ}£?ŽZ¯P4I¼?‰Wó"ðv?Œ¨S¡ãì?'Úù+°‹Ó?r©óμÈ>?ïîjse/Q?^Ð౿»?Mw/ä&«?%¯à}?a@V¾Z?^fõÂu(53FGL J1018.9-5856@qŞ 3玿û
¬RÐÝÀ6ϽBNÀ9'¤g¡Ð@lá//m@
ô܄¥Á›@òƒë‡x¿Ù£ôüÁ²¿å¯íÎ¥!¿ç¶%÷
ø¿íTš\78OTHERHMB?0?q‡kI?0˜ÕòOA¶?íg!Å'?º
ã ªŒù?´¶²f ä?ºÃه|8>ù­Àq¶è?(s©i3"?î½Îð:·Z?¤'Ѧÿ?¤ÛDFS‰?¤åæ¡3I?–å{»øÑ?"Ð}³þy?èHÞf#]¤?¶¹™PhW´?ËÿÖðJU?µMÂhÀa?<'Ò¹?!¦é†ð™ô?í1ÆjR`¦?©}‹‰º£y?¶jý‰)J?©{HnWì^3FGL J1020.0-5749@q½ž 3玿åeSßÙ¢|À7¼ií£ùÀ9Ñޜ)¦?ñØ$ ñ')@Ý‰ˆk@¦nmXž¿—?¨®×»¶¿ç¶®t¿g¿ä1yðºp\¿éc`!¢½PSRPSR?w'8–ªl?v¶Ò°q€?–ÜüÖ³Z?Ÿï@úºiA?ïó¨|?¡)Z®"?'ñöÀ?žd1$ï?³7t›ð†º?®Æxë¬~?íˆ"Ò>Ì?²²hSŒ?¯a¦|´	?ŸÝq`ï•?º{îÿî?¥T«¯ ×?êºgÕ¢ÿB?ª¼òmÄ(í?·>_¬LI?°›d-҄?£PŸÝz4?•SÓ…›V?ëåc*žÔ?³Tlèki¹3FGL J1020.0+6323@bK^?»×²@G"_£Ô†À:+)­xs¯À<ìÀˆì?ëó0Ùç'v@
c~Ì
à@Kø`îW?î×·¿D=¿ä^häq¿êY4ð¿ä|#È9ȬAGNbll?é#³l}?Ë)*y
?ÉÛÔkïy~?Êû@gßÁ?‰}Œeé!X?'Á¯ñkJ?è¶ëà[pd?Ê)ž˜nKË?È`°Ó³€?Èå™D'?£öú+²?¦YƒO?ëüvë…4?ªÉ¥øÍ?´­''£]?¥jª2g…§?­¥Œ"?—!¼fMÒ?ÞhŒu%™h?È$ü]\áz?Ü̹s'¾?ÉA`žô?³*ç雏]?²Ôwu'W»3FGL J1021.8+8023@`@Iÿ'ò¶@AKg€AÙ¿À9é-¡"ú×À;ù/À·ë"?êÀû1Ühn@_ih¤Y;@!@—tѿ吒fõW…¿ç—nµÚ¿ß9,"ç
ï¿ïÿ±žs.AGNbcu?ç£Ñ*2Ì÷?Íl\Æóf?¸Ükûö?ºqþœ|?Å…uWG¬?Êy'DRƒŸ?Á\jö¼¹­?Õ¤Gë‡H?éŠ@ägƒš?ÅÿdBN,?°õ"ïJoØ?±à#•o:?é=›_Ù+f?®#©~¥Ó?¾oªÍâ?¦¼"¨‹z?¸'‹Öî? Wâ'h7?Ø÷áÌ®m?Á¢äwõx?àuÇZ5sï?Ä6(§?¸r>÷!¦Ô?«Â*ûN¥3FGL J1022.3-4234@q<‡¿çáü@(š"ÿ%ÀÀ:Au}Zž²À;¦ÝÉtR¸¿æ¼ ÜGØË@Q®Ÿð¡@° M¼¿é‡wÏU¤]¿ãÓ?
_ˆ¿ãn,\€¿í¬"Ç
Ò'AGNbcu?í!ƒ.ä?·pàU+€? )ÚZ?°QM"]Ž?­â=ò··N?´D,ê²F?í"þÙ«J?³Ó$/¦™›?†wûÏvj?‡¥S˜\)?°'+Á3?²lûÚöÏs?êï§|å3m?ª¢qj?µwºK›#Í?¡_ø¥«Px?³	Í;@Â?žûKºSͶ?îSVDo?˜iUש?s1š7vA?qwËjD/J?¨Xõ‹XÚC?—AëÏä)a3FGL J1022.8-0113@n¨Äê@F0³ß•ý-À9#a.AÀ;p×%+3?èp/¡òóA@-hì'°ô?ýþjaÐp¿æ—ÿW?ˆ]Úü^ݿ׈ô'Q¿äö­Þl~ÑAGNbll?ïG~"-û²?š-°=uo?'úAž+·ò?Û±\&D?‹&–U[x?"ɯR°7?íÑ~fM?¬FÍy¨½?¨À`ýIMë?¨TS±§7O?"Oq;Éá¬?"|h=g£Ó?î$€¶4Jq?˜ð·Æ…T?•Oõ>0Ú#?†2š¬¶—?£ùý¢ëæ?'¤ogX£ø?ê[S/=ä?­¦çѥߍ?¸jœ=X?¨YBَIh?´ºÇ†I†?£±…c«ü3FGL J1023.1+3952@f—|€"Þ@LlØà†8À9ßZ"‹ECÀ;䇀'a—?âk¬D}C´@~P¿54•@ÎÇà(õ¿å£€¢Ÿ5¿ëËåŠø†¿ïþ¥l-:?ïȧèMAGNfsrq?ïýƒb@eŽ?6²tŸ&yû?þàEPÖD? MPm{?(ÊkÖþªŒ?2˜¤©Ö³?ï·eG}?}ƒµ¾?hpèy£
?tɅ‰©ÀÏ?ií²>àA?nÐÈÜ΋?ï_»þYþ~?"¬d
ÿ-Î?w‡-&á'?q2æe¿ô?ŒMiÖ˜?'zÉ%¥Ô?ïõ9zvì;?e†¾¦ÎPA?å¡#¾‡?2pߓbC!?T,¸JÒ?e6
´îÈR3FGL J1023.1-5745@qÂÉ?¯Bx¿Ù2ÿÔ™À6¢0'åøÀ9…{2¦Ez@Ïnc¨@܄¥Á›?ýp؍JUå?ìõÒL–S¿â#N+\$C¿çæ+¿1¿Ò¿ì:Õ_â¥PSRPSR?5÷û"ÞkT?5ng]VhÙ?éR|ƒä‰'?ǐƒߊÃ?Ê«ò«l.?ǎrÅhà,?o¬RŽìó?85¬äk¿??é`v锵¦?ÃçBGJ<í?Ê{Öd"׏?Ãç/›_É)?k>AÉ<©'?hüèÔÜ?èV™™ã=?·ÉP­vB?Î8 "k€f?·ÅàKÂ)?DÊ»é3ÚD?FèB™Çn?èWyöMå?¾Ä°ôôƒ@?Ïá×\=""?¾¼6i*%E3FGL J1023.7+3000@hÞeÀ¹™@LËèÀHZÀ:‰'³ò
tÀ;Ü&¯—1à¿ÉæM:<ß@
cäz=ˆÍ?ûîþ?áll¿è㎘';4¿å‰}AR¿ÀYå4ÞÀ&¿Ò§¶|d'AGNbll?ïïù3Kñ?_†¤'õ?*O¼9ñ‹o?'5þ{iõ$?\ÃÌ)ì?^_0€ƒ<s?ïÇQíÅ?}YíL:?lï·²G;‹?sÿŠñ¾º ?k÷ö_ó±Â?o	GŒ?ïRH'¾|4?€}#6>¾|?}+—Ì6?pŸéˆ
5?ŒãàDz×Î?x,¿c‰(¨?ï¬ê"³¼?{-ÑaSt?/Èý/ñ??sVŽä5=?"F7#Î?z…m:'3FGL J1023.9-4335@qIo@_k @':¢?ZˆãÀ8Ȕ¤gRõÀ;ìþ›{ò?Åëô
3î@¶b®ËÚß?üŸ[à{€T?Ülä¸Y¿ß]"–Ž]¿ÝZYOº¿µZeÞùlŠAGNbll?ïQ»ŽÆÜÉ?–'â>Ô¾á?q\ÎÒ¸¤c?ké8E?'qZrv=Õ?"Ööž-è`?î"grëO?¬u!|·?tœÓÍnz?wè-ü?¤.UîW5?ªãJÈK?íÿoJP?¢,Ç
üO?›ä^¨{º
?ŽH*[)œ?°¥ðZf¿?ž_é—<ãÔ?íx2I|?¨JˆÒŠ8è?båS_‡Nû?qkªív"?·5Ò»9Ÿ?¨#¤ô[;©3FGL J1024.1-3232@pãrà\̊@4Ðï 6kÍÀ8¡ÃPLH®À;uÝæЄ?ó•xÕ©À-@¦mV½@¦L A©n¿äŠ«Áå=¿çž9='A§¿çŒ¶@],¿æ::×þjeAGNfsrq?ïÝ&4.#Â?ªôËVÕvš?EþH5ìüy?Gl#"Pm?mZ9Ä`ÿ?ªø7ÈÕZ?ïɕfD»?{Ãs{Qh?cÆVȽ:?gL:7Èb?qS‰ÅyD|?v>È%ãþ?ï¿æ¾ÚË?I"³º?ˆ²9Ž¾ÃŠ?"PÆ¿´8?ÝÌÁŠ‰×?…Õfõí{?ï³p˝!?"ûï® Ù?Nè«M1ñÊ?SŒª¾›äû?5B‰˜R?"hèeí"3FGL J1024.6-0718@ouÛߏG0@DB+ ?:¨À:Z÷xr¥À<J§Å¬G?ù	ùé-@5ò1
d?絫ºrF¿íqTsD‡?êÜiÔ¿èABah>¿ïÿ­µ/w<PSRPSR?¸H4xˆX?À˜@^GȔ?ìZ;K?ætfՎ?"—Ͻ¤?±ó_® ‡?¢xd@›YE?¶¿éþØg?íÓ¦?½›Ÿ‹)ªb? Uª.êEÈ?§{¤=!
?Ñù¼E³"å?´ð91YmÃ?㸢!úTQ?´×¦½ôä?ºSýÙ_
ã?§$tžV_?ºV‰ŽÒªÃ?ºÚh÷]í¨?ìˆÛE֓:?¼`šVµÛ?v)Ä'‹¶­?†€aR'°É3FGL J1024.8+0105@ngààëgÃ@G$:`NqÀ9Ýë˕•(À;¹ÀI0Ëz?ïcV†Ê_	@
ª£¶~â@d±€9"¿à'…gÏ¿èåÍ-}¿ìK9ðø·H¿ãöÉï!áAGNbcu?æb°eL¿®?ÌxA6àg2?ÃÁ¯¨ˆ¶?ÎÄ9ÏFT?³h$x'?Â1m"î}?ìQ7`;D?Â\»bh—Ú?·t"ñß?ÀéÊ‹.?™{CpñD?œsßýMº?êqyyVnâ?ª´¯·]/+?´@9éº(p? z‰«CÀ?¸3úK'`w?¢v/3µÏâ?ákpâô'š?Å	Å2z¨K?ÖóoÑÛ?È
ZÆÞ3i?¼ «)Væ?²Ä]^ÿd3FGL J1025.1+2333@jZe>‰©@LoüõŠÀ:"ÜޓÀ;ã÷YhQ"¿ºþãA@ÉAÂUP@™ †¿åÞ¡ï\!r¿ìqz@¸Ø¿­xÕ~]d¿ì{¡ß8_BAGNbll?ï'0 ;cy?"Ä›õ¿?f­	Ú\Ô?k¯§þ=¬?†'.°Š~?"šp¸ÖՃ?ïVHN»'?›q"‹X?'
nêÍÙ»?"¾*KB]ø?ˆUµl?ŠBuäx?íe¡"Ðâ? Ãa=Ë? Üp'î?'Ìz™2yà?¨Ò%á§Éç?—Õºsڇ0?îª^L‰™ï?ŸPµn÷'?v^ÞÀ»ú?zÄ0àÛ?¢—¯[ŽIy?œÕíì53FGL J1026.4-8542@r®€{»bÀ7¥pà<ìÀ9Q½‹ç)À;}«Âßä¿åtªÊ¢Ò@
×á°ß†c@\à*͉¿å€4$Â#ž¿âB÷ÑÕ¿Ù[$_AY¿Ý»‰-±éAGNbll?îÃÈÂò¹?¨Ãòp§#{?Zçœc½+`?fž›ãoëf?¢ì6í¹?¨ÌRó­?ïzÔ?ýš¨?'`Ø!´á?hB²©uŠ?r"g¨ÖÑ?‹:CV<?ÊÀ`¢q?í¯|¡ãŠ·?œÿi‡ÁG?"ˬï|3??"¿{5?ª¢_j	:ý?—!䱍h?îc'?šibdŸ?G†Õl%b`?H…Wd]²?®««§Þ	?™ùâät'?3FGL J1026.5+7423@`ØÑ Äe@Cœ¦ßÓ9ÎÀ:Nd!À;ˆºô]4Ž¿Ý·P‡4šÅ@´A€}é»@•= t.¿èΙ«7¿ìó?ôüZž¿Ä
‰d‡¿çÍRh؆"AGNbcu?ïÕ÷è´_?Œ:‹n]?8¸7ð¯?7/©¯ò‹?sꀌ¥?Œž‡¥f?ï¡ÄíZ_?"µý­ßÊ?v;›Ù­'~?uÑTÒdM%?xáíyPN?}Ž"Õ@é¹?î˜Fzˆ?"ül,~?†ã²Î+l?{,Ècs? ÅÏÌ©?¹Qû/ï?î£Ìh:Ì?˜uµq(r?M ÈË}÷/?RðU@ ¿£?¥N¶\Ž[h?˜GHñƒà3FGL J1026.9-1750@pNÔ@(äü@@\ßÔçNÀ8Ÿ–/ÍËÀ;,WvßZ?߶ÞÓ#lÛ@}ÙõI?þ·ÖÁañ¿à]ý<½[ҿ܀¯õó¾¿Ý!+‰E¹s¿Ùo¸ÕOAGNbll?ïûÖ¥~îÇ?;~Ôbcù?%OTx…JŠ?"[VûPn9?6£)ÌG ?7ZŠ%ãæ?ïÎ~~z&?y
jßê¨?eԛ¶è\Ð?iÞ¸Ú÷û±?k¬æ-}?r2‡¢H?ïc4}4úQ?rô/hñu?|¸¾Sè?uڅÙJh¥?ˆÖŸÓµA£?yaòÒë?ï'.¸Ô`?Ê1¥\÷Ÿ?1œh Ói?5±˜k
x?ŠìÑʁ‰?©ÄÍ^[3FGL J1027.0+0609@m·±~þá@Hç3çüÔÀ:\øÍØÀ;ÓÐJ/Îû?×°ý˜G@¤H"Xšv@¿¯ß/j¿ïòýý¶?ÍHਿ犋¸k¨¿Ðqþ4£Ë¢AGNbll?ïÛÁžD&Ï?sH÷»—¶?j¤TT‡;?pç#IBe*?T{zÏ	R1?VTéôÍo¾?練‰Óƒö?†Ó'¤ð1/?z"/­zÖW?#­Õu|C?r0‹hÃ/
?u]å —?ïü™Å1p?žû=çjÅ?ŽÁßû©¹¡?†ƒcü0Ý	?þù"	ê?'åÁ5ò{?ï7!Œ,?'ï¬L%g–?Žúðo·¡?¿;,U«?"4üÊí=ð?ƒ5ëÚSy§3FGL J1027.7+6316@b6@ Ç@G€8_ÂÞ7À:s­]èÀ<)Ó8 Ù¿Ü­öaµkv@…¤ƒWÛ?ÿïkˆ±j¿ë¹²œR¿ØØ>ÚJ'°¿Õس#È ¿äÑ©u¯¯†AGNbll?ïê¼ûè,?'À'ÎE›=?`§>\ÈP£?'P&¤`$½?BoA>
R?K4¼Æà3?ïPÒ3¯p?žL­wø¨¿?".üÁà‡?˜Ž±˜Ià9?…ÑïSìñ?†6èµ9d ?ï5sá'Í?…h³Å²?…~p±Ã?~µ¾'vw?!¡–é‰À?wõhÝä\?ï5å>³uO?öiT–è?v7þß©ÄV?s¼JNbºz?"µXq¦å?‰ÃãÀD3FGL J1028.0+1829@k}ì_9K{@Kýfàé´À:_—+*P6À;ìRb£cG¿ù÷aüt	@Ǚ³oق@ä]_šÊ¿Öž?ý'3¿è;h³Ÿ_¿ßåå¼þy¿ÕÚÊPñŠAGNbcu?ïðöz—î?]f§xØ?<>‡¾\Nº?<À¶y§wc?Xàq9Ê?ZçÞx^øx?ïز/f?tòfÁ9b?cñþ¦Pø‰?l©ùE«£1?cþ짢?fAWŽ?šlé?'ÑH$þ°?oƒ<ˆ?†í³"¤
é?™.~i&i?‡‹?"ä2h?ïåá¨ÕY?g¾@›:2>÷ýiŒªÑ?m
èu'ù?jÁ#"R¡?g´¨µPíë3FGL J1028.4-5819@qÑÆø¿ßµÿÿ˜ìÀ6ØSéŒ À9Ï´ÂêÌ@yuòËd@1<¸íó@®†‡C*Í¿É#»j"‹|¿á̈&œ'¿åé7ðS²¿ëÂθŸOPSRPSR?U)^?mô?U¯½Öۆ?ìSw_ú†Í?Á
$T'wI?½Z²ËÌ?Àõ•£5Ê?)#úÍél)?Ub«î(	N?ëÜv[Ñ?ºîÑ6Ç?ÀëE'ÝA[?ºêý[Í2–?'wâŽx?‹ù¢þ+û=?åÂzÈymw?»i¦{?ÓY¢ðäC[?º›gE}"?M K/t]¼?Mʖ}6Ú?ìB4áÀgÍ?­²ÄƎ?½³[ØÚ?­~.á&Bê3FGL J1028.5-0235@oN ‰ãC@FD!?ë¨ZÀ:^ÖÒ	L°À;՞¢ŸÓ¿Ü=ȋR6·@½;¾	;@9Nª¿àÛµ7QGh¿çü4Œ'7†¿áðzŸß¿çp¹Ô«*AGNfsrq?ïübא?E	›i²B?¦åSw¥Ï?2Â4Â*5?9;/q?CEêOüéÍ?ïËbiôa?w¡#ӑù?i4ä
è'W?kîCú å?ki‹#
é?o†ªSsI?ïXËçf4—?ƒÜûëÝz?xê7L:øæ?r…"Ũâ?Wê€U]Ã?~""¶,_ò?ïÉd"DÕ?t?¶÷1åG?1/øÁÆ@!?-Õ û!Þ?z:þ©Á1?sÛ;è,ië3FGL J1030.4-2030@pz-••@?eþßnÀ9¤ºB†MÀ;~o09ƒ¯¿µ*ÍóŽ8°@´ìL™á"?þ;bŸ1‰¿ã
]Nd¼î¿àÕAêáÇ¿Î?©˜5Á¿àkÎZXAGNbcu?ïóÏ5¼?S1ˆ8a)¬?:Aa
-?5ϕŸè>–?Qс¨
?PQ_‹–,&?ï¹°šRÞ×?|z™vy|½?mí)ÍÐÂ?i)Gª%?t™¼A©«ï?wEuâìïß?ïW«p{k?€>€÷ ð?{7q?Ÿ@?n+o‹öªø?Œ"ˆ(|²?yÙM"Âh?ï#1ׁ¸W?ŒV›Ú{Â?HÛi`!ø¥?MrvŽOÍü?šÒéÄÇå\?Œ&"Þ	3FGL J1031.2+5053@d.%¿­@K7èÀHZÀ94
ƒvA¦À;UÊÆbP¿ò–i¹W$@áë#$j?ûHŠàï§?²ïâ{ŠºÚ¿âÝoFVH¿ÒñŽÈá¿Ífl_hŠAGNbll?ïäl'"'V?m,Á‹Ä´W?@ª%ï7€Z?@Úæb2?ghôb
ÊÉ?ko15
î)?ïÎnƒ|@?{¹Ü5n,Ü?göÜ!Záâ?rè`@n:?jµ[(Þ£?pÖ8'ÑÄ<?îe"]¥?"F‡ÊCÓ?xº?Dó?'½ú4uV?Ú¡ukF?LÃWõ(M?ïCÎҁ'?—lº3? êªÄÿ?2€ŠÄo£c?—eðøh
?r¨s¸Ì3FGL J1031.6+6021@b"àç6@H›¿çáüÀ95?VW$ªÀ;UøZ?Ç% þä@	1í]ç@	?n)ÿ¿è˜ùX›øo¿çpØæi3©¿ÞµÕ
|Ú
¿í/ö‡,AGNfsrq?ïëöÁ/½ë?…
ŸŒaí]?Sê«`‹Ô?"€Å»m²?T'ýõ#Œ?bºì?þF?ï¹ç®b´½?']oWf?r¸Ê¡1[ª?zG¿¨ƒw?pS^-tE¯?sqT
†eL?íë?ÿuM?žTâ8ƒú?™·¿`BÒ ?ŽíÿÄgç?¤p XŽÍ?—Æ#±"?îɤM€Ù?•ÅÍ8,?aÏúû
Ë?cù	«À\?¢H¶‰8A§?"Ú"X6pô3FGL J1032.5+6623@a»/ÀL‹Ê@F¦>ÿðÈÀ:ìÕy(
À<MiŠÞô¿Çæ²üìû@A'Ž³6¤@2o¿¨Í¿êÚԊ¹àj¿ÛâîwAý¿åþR—¿ÝÀÖw¤	AGNbll?§p?¬v®Ø¹m}?›n
WÜ×?¬5ÿ¦ò?QÛÏ3R¯?[\@ã†*÷?ï¶2n­1?ƒÁ2‡¹Î?sƐƒ­$?€êo™w?q 8•ã‹~?r"ìëŠ?íûKP?£"äCñL?©ê~ÿ9T?£Z'Dü1?‰C'ÆÎ?y/Ñæ?ïÌ3¶Û´?t®cÕæ)?VÐKÈl®v?V‹ðíØ?t2 Yù?qÀgb¢GL J1032.7+3735@g
Âß
A1@M‡9á£À9A§~^ª°À;ʒ~e'¿í!ìè0"@Rk~SB@™÷?':¿äìðgAéÁ¿å*<éâ©¥¿âX<'ß©/¿ä²T²ERAGNbll?í6TYÞ®l?µTF)dŸ2?‹		!/Ɋ?ˆ7°{°ß?²ì<ä"s?´ãþS"%?ï2¿f/›!?£ÊyºoµH?âQ‰žý?›G1hÁ?†ID"˜q?'íÚ¼T?ì¼æò+™?¢éèL}Ԕ?žÔjÆÎ?ŒÕœS†§?²'ST"ï¶?žGÞ¤a7?»ÁjG?ž,xËAí2?y˜ò"ʳ?€ ãwÃ?¡ÒUóeâA?›tóŒ=3FGL J1033.2+4116@f+zß.Ï @M2R¿ÀtÐÀ8áî¯u£ñÀ;·uª§?ÖLž?Vé,@à Áìt@'Ð pË¿ßa£½‰ä¿çB‡ÜOC¿à<%ÿ²Áø¿ì#ٍiNgAGNfsrq?ïäÁÈa?e-é´ïñ´?RÔa;ϟ?P0DX<V'?b4ÍmÒI?b]£^DEA?ïyØ­b?Y‡RÝ]ë?'…øº5
?"¾¼"5›a?~d"5käc?4Y&j8/?îXd۔­8?˜"!í¬Jž?›WÇè-~B?'K æ‡^?™›œ¥<ڐ?Ð\Ÿq
?喙¥¼g?—»nf?ñ¢ƒ*n;?'©è ¶ò©?–Ñ÷i³;ù?"JÂ¥¬ö3FGL J1033.8+6051@bxæÿ}ú@HŒö@c^À7Ç9k[˜­À:Ñ«ì'tº?úy4I]Áý@æ~ZÎؖ?ÿļ'ÂåÿÙ蘙®+;¿âÛÆT¸"¿ä qFŒ¿èjó®AGNFSRQ?ïîŸ(B?g!u…ƒ`?JbõOìÈý?V*DÎÐÒ©?VÃG1¹ ?b‹²Æí¤×?ïØÓx&Ck?yÍœy?c7|G"ß-?nOWíË+?cõ'7¶?m9Ò
}b`?ì³eÇ¥Y?¦°{É×Cü?¨œ`˜U+À?JPFâÁ?¬-F[0~ž?œ¿­[Îû³?ïî……µ?n\höcŽ÷?ž'ɏFù?)ÿXI©0?a€ªT
[?n—'µ3FGL J1035.2+5545@c?ʞõ#-@J/xßå®EÀ:*ôœõn­À;ñ<¼HñÀK|7³ög@Þ/â+Y@‹õ €"Ž¿èe~Ñ[¿¿éöíO×·?¿é«k¿îøË1}bAGNbcu?ïû"èÀÏð?QÁ]™ýó?1(}
Ú4"??ÓÁòmõQ?20<î¦Q?MŠw»Þ?ïÆÔ""î¡?tøŠy?m5à&e³?vIù"–	×?kõýZêø3?u"Oœ€Ø?îâ_½3\?"zôÊæŒ?Ž¼ry×-Ã?"K¿lh³?"UϨç;?Ð¯ñºð?ïÞP9ZF[?uÖàËmì,?2†uþ¾œ?\¬ÿnÌ?o^ø¹Í?rÔYÈ|«Ì3FGL J1036.0-8317@r®½_ÜßjÀ5O_¹£ûÀ9àG­=»LÀ;®ygÊêt?ê÷6õé@
ùpò[|¨@¤H©hš¿«_QÒ¹(‰¿æL!·hj*¿æö}‡-Ì¿ïÿ-zYPSRpsr?é$Ò¶Ìï?Ãk×>Þ?¸©jïÏ?*?º;—À€¾?¾66zzYb?»äåLf$?ÙïÃNµ1?Ä㍍
Yî?Ù'ìßvû?Ä*`^?ÉП£§§È?»‹Zƒ›îÝ?è»×M°Z]?­…ù'Y¨M?¼´vÇ{ƒ?¡ŠôJa²:?½l¸µ±–?¤ÞÀ)b9?Ø^ÄVâqb?¸$¢âÂü?Ù䝮¡SÎ?»fSuBÌò?Ëy;ôøu£?³«!{Í3m3FGL J1037.0-2934@pî¼ßï¿@@8Ïà0VàÀ9¢<PgÀ;‡vG…?ï­Ýò ,A@δMÏì'@½æ¿Þ}ºüüщ¿èGL'!L£¿äŒgv©!¿ïÿ =Z~AGNfsrq?ïõ}<{ð?Q6mbÏ?AX\è/5?A³SÅÍú'?Hݲ±(!?G™*7ÐÝ´?¹uÊÝ? Ð¿¡¦_Q?˜…žÂ}ó°?˜@™á6dˆ?IêÈ°Å?'½Ú®Éiƒ?îC"Aŧ?™× åP?žý襁|z?ŠØIÑ6?˜ž¬
δ?Œ¦X
ä?ë¼ôþ,r?©9Oφí?®ûËêÇg?¡—»PZ€?²¡Î8¹?£Øc©ý%V3FGL J1037.4-3742@q9Ê?‰'Ë@1òŽ AS‡À:*®í¾´ÜÀ;ÅÌðÞúÍ?ÕêêÞÊj@ä4i>÷@
îßòŒ¿èb^<¿æ/Y^ëô¿ë'lkZŽc¿ïÿ9M(¨AGNfsrq?ïÉç'ª¿?y\"JÅÒ?p¯ÉàfO?u(vóÀ P?eï‹Ù"u/?hìVŠÃ?âg¬¡¹Ý?ÍKýA¿:"?Õ
©tEiÕ?ʝ>¿üõV?¸—õ!p#?¸)•Š?ì¯`ڂ¡?¢i½m"‰ÿ?¦Ò=zóõ?'AC½%0ö?®7´Üáù­?›è¶Ûø/?Û?-EcúË?¾­3ÑÔ$?ÜÕÕ6
³î?ÁèÛ<þŒ¿?¿«ö9E?­¦ÐÈ¿S3FGL J1037.5-2821@päo€Uûµ@9☠uUíÀ93Ád¹½üÀ;€C_?ÒïñŒA9@Õ Û,a@ñºÃ.¾¿æ8÷׬=¥¿åáJ‡°Œ¿é®÷!F¿ä"\@?-AGNfsrq?ïùåêL"v?Efó'Iz?9múµ)Ě?5¯];þär?7b²æ²'K?>d:P¿•?ï¬Z‹"ö?'á±ËÑrï?q©Ë] ]"?p¦»'A~?x(îØd™ö?~=¦@Dáï?ïVdZaU»?"ƒÐ: 8?z¿¯B­?sƒ.³hq?ىŽ?€"þ¹äV$?îÍl¨Ú?"äMšŸ÷ó?x`Ñx?Çã?sõ´òÔ¼? "vyx?"™Ž±j<g3FGL J1037.5+5711@bùŸ˜=@Iáü`8NüÀ8<ÃÕ­FÀ:èâï?õ.HËùp@¡½Gɘ:?ù!†â-\¿ÓS'¼Ä¿Ü,+³sE®¿Ù[žÔA
¿Þë·V¡öAGNbll?ïìt–ˆõ?n?†ò£\U?81ZÅ]ã?Dëp¶?`…>•Ó`-?kw[ñÏ¢?ïÂM÷T«¢?
+âD~'?p¸…$§$v?vê©òšÆU?l@þbk?p˜Û"«.?ì|d§|Bú?§*Èç_Øj?¤ã"ÕD8¼?˜ü4íi`÷?±«Ù{ËÇ?£,ƒ+Kƶ?íÈšÎ֜?¢}™Ä•T?
üF­I?ƒ2C›Wþ©?¯žÊR ¡?¡ù´{ÎÙ²3FGL J1038.9-5311@q¼ M@·o?ÓՀÀ8-¿¸èzÀ;)iϧr ?úÆbã$''@F5‰ÏÍ@#Qv?Lq¿ã¤˜";¿è@;ªóV¿ë'ÞFz}¿ïþè"IŒwAGNbcu?ïƉñA?u3ïP±Z?gÚ÷pkxJ?g¹ÍMœÃ~?q¿¼Q¢µ?ngÙýÝÓ»?î'öŽ/™›?°]û´§l?gŽìᘥ?ráŸ,è©?¥g¨NìÜ?¯´AwdÈ+?ìª
œªfœ?¥&(Iý¤x?°ÂÄޝÖÕ?¡'PÑßä?£ÙÌxè¥?–MÆ|0p?ïÛ5Eîž??v£Åvç®Ý?EWO"™ç?]XᏢ7$?otó=|šh?u%'•Ÿ3FGL J1040.4+0615@nXà†8@JE»üÊÀ8Ñ:6\³_À;x§P;¶?éq‰žò@OŒ¼çQˆ@ÏgÀƒ"H¿áø~«E'Z¿ãõ1Tƒ1p¿á÷,̑é¿èÑ2uÚAGNbcu?ïè13\ͧ?eü©.>.Õ?PuŽP¸?KðÆR3%?_(€¸Je?c‰—~ <à?[F?†×œóËjK?}CjJú&? óٛUŒ?wvh(MþÍ?xAö2°_3?ï4‡Ej3¨?†ÃÊíƒ?'ŸÞŽÄ¸?z9hÍ"¨?(W.í?îDç¸?îÕÙ4°»(?"ß}ç7+ï?"cý)«û?}žê1ÒNÌ?›Ú՝5?"­ýTk]<3FGL J1040.8+1342@lÄHS'^@L]⟜èÙÀ:¦–À¡E`À;×Û©¢f?Þ¸4r@–`Þg)?ü(ôÀÜ©?íó™Úç¿îö'LdÌ?ë@"!'÷¿¿Þ «ˆìAGNbcu?ïç÷Õ×æ™?}íÅt5?P–À<îÒ?|.Nk†¨?_zHõßf?e*ëË2A?ï¨ÅŒä?ˆk̪²cå?v9«}֌½?oíÒ+?ucŽ ¶?{Ù ­õ[Á?îÊNÔ¥QØ?aÆ6ÍÆÆ?"ìII8?x<'ÍéZã?œ@œ±)<?‹ü:Õ¤¹K?îßŽ\?¯þè]¤H?F|èÙG%?d…ÚaW6/?¦Ôá»óµ(?¯÷
U(­ù3FGL J1040.9-1205@p<>_·¼@C͆_¡PÀ:_Ü#åHÀ;×m‹ô•i?Ù)EÝô6@s¨(}¢˜@ÚßVø4¿ì	uéªíÄ¿¹e'»ež¿á`!œn¿åÞµ'ƒSAGNbcu?ïôdèG^?Q{øCô¢,?K!œþWú©?JS¾4k^™?CJÁä/¸2?@»"–:é?ï"K;ûÒ!?"¹¾f'"?}€iù6H?z¨VO#{Y?y@ᘸ§?y`Z/
§¨?ïaŸOïþW?…*¡{èi?"HMŽ‹]w?€ '²JÍ7?ƒOÞuu¼?u9j@Ÿ'?ïPøœ,©?†œ.áƒÌL?'(r-«"Ï?vò­.W?‰™fÇOr?€ Ž1aÈë3FGL J1041.8+3901@fšž`=Wy@NGU?ÍuiÀ:Ò2Ò»#WÀ<]€
×Y?âUÁݧÝÌ@
÷œ{?ÿ'dÿ^'?ïþæj­ž¿ÍÀ…¿z²V¿æÙ«<%¿Ü×k\fÖAGNbll?ï©0<°y?†Fõt'Á?'GúIjn?…@Þ(ÊH?]mFÍ»n?`$¤'õ~?îßÜ[âÒ?²·c
Ò͍?¥ŒâŒÐì?°eÊï'K?'
?Zá͝?'Ø-íú?íõÙ"|?œxHñÀ4ê?¡Í$Ú+?–¾DßgG?Äü«S¼"?ŠG8‡U+?æhk‰j·1?ÆY‡Bd/?ϟl'J?Æl"™Õ`^?ªû"ô·dŠ?¦˜Î ñðê3FGL J1042.0-0557@oֆÀ
¡©@F:ØÀ  À:kÃ
0j+À;ÎÃÍIÊN?òi´Ï€t@
Í."®×?ÿr?7£Z¿êﴈ³Bb¿èJWqMl'¿¦ÛnŒ`Ý!¿ßˆùiÊWAGNbcu?ïw¬ßÇl?"Ò[¥êøB?{vˆ}Ô?'IúÛ6žÒ?"YÅÊ¿U?Œ–ZóÓ?ï,¥–¤?¢ö):j?'.hTˆ~? £*ðô?'ÙyÉÔŞ?‡T·¶ï?êí~sÇEÏ?¬™Æ	lY?µ¯ a<Wˆ?£¯"Pa…?²äì‰z?¢qîÆN*?íé'ï×H?¨	mx¥"?Œ#0¥mB?˜SÅ­à?ªdÍôÙ0&?£kzI‡Ú½3FGL J1042.1-4126@qf1Ào@.cŠ '§À:˜PÀ;äcâ'§å¿û!tïÁ@b=OçÉ?ÿž/ÀâÞ²¿æÃڈ!L+¿èiòX]ËH?½ž‰`™üI¿åë®ïí
_AGNbcu?ïÜy=4D?€Ó'ÛüO?(xÏKK"?'i\v
x}?pÿšÅ
šq?€¢'™CY'?ïT;Hò$?¡ž'È?cáy8] ?j_»áàLN?")oßïþ? ôQéïœ?ïê3¤‰˜?‹Ñ5Y!‹í?}\Æ·?pMîô §|?•+¹YÁ?‡ÀŒˆ+,¦?ïÕ8œd!?r'çé±Ú­>⊆oØ>öBÉr¸?uZlÀ5·S?rŽ­|Y¡$3FGL J1043.1+2407@jsˆ M@NÝÀ:SÀ9l5Qñd\À;²£á8k?å-ÇêB‡@"iÞ @ðO@Z
=¿ÙÿŸØwûº¿åSâì&Œå¿ä@½€­Ã¿åŠRĝÿ/AGNfsrq?î¶É|E®? 0ºÛ$?—þ€_Æ?—>=á.Š"?'AÀöê—?'¨DӔ?îPü »Î?¨~Ï÷û"?¡{õR)áˆ?£]n€½X?'è}"Ã7?"·¼)Û?íév¿Û?¸?œúT€#âW?›uWÛh'c?âsüe)?£­è—»à?'4xØP?ê&·®ðd?°"ºåÒ>?¹Kp _µ?¦ù+"7=R?µƒâ#h6?¨lrÛÁwë3FGL J1044.4+8058@`I¥Ò@AXe_Ö)mÀ9Àû¦ÔëÀ;\íbnŠ!?î3€FêÜ@™¬Ÿ°´é@"ÀŸAú¿ØEÛpBw
¿ë$¶-ׇD¿ê:` |!d¿ïü9®;VAGNfsrq?ïüvXQ?>hså6??5'e­ "#?7ó£îÄÉI?#Ó@9Ã4?,?üþÍ?ïZ€jC§?'aÁ
ý"|?†j§	ð¡b?"s¸–â?'õ>e%—ç?†
ÉêSŸ'?í?
—ÚK^?ŸG>v/¥?©˜À-…ó?—©qZÝlH?¢½Â-Ä?"îÅ3ùâ/?ë}` @Ý*?±öÿçRˆ?®—(«jݍ?¨½M¿'¤ú?´Éj¨C§î?¨˜‰²Õ¤'3FGL J1044.5-5737@qé2`o¬`?òx W À6·èɂ•qÀ:BÙ­…ߨ@z—ì¯@aP!«vf@~÷€—:¿ÞÀõ0̯¿äT]ã
%ô¿ç
€û¬Íî¿î‰ÿJÉPSRPSR?3ŒQ©åU'?EÖ»¨ô8¡?î®áîó\?±Y·¬ ®?¤êÈppÿ"?±BÑå$
?2.‹;"ý9?I,Ewú)?ìܑW½Á²?´{Ð5Ús´?¹	F¶Ö]v?´:GE?"­A-1¬?©,ŒŒuæ?è½-œÈi‰?¶C}Ú
À)?Êu¡g=ó£?µÿ6·õ€?P>º¿?OÀvóqå~?î´b\¹?Ÿ´ggb+Â?®rÉ<n»í?ŸH3÷Q»ð3FGL J1045.1-5941@qù±_ˆü"¿äB% 3ÍÉÀ6´ýÓÕՊÀ9­Õ~L69@z§3
C{@4ü(+?ýÇ3½G¿Ò`x:Ï3Ú¿äÆëvÛÿp¿äˆ§¾öJu¿ç.†%HŽåOTHERBIN?hš³" h?®ÈÊ&¯Û?²»¿Yë[ž?»ŠÂðÛëQ?íía/t?»¾Ù~ó7?;Œ¡J<Ý?SÚ©Þ?Øý†‰ÙÐß?Æ2¦éùðß?ã}Ë&ï.H?Æ:xÊ°ò?œ¹˜ôÊÉu?'Ñä¨à
4?Æ4ttQ¶?°( >Ë?é0¼•F?°ú÷ßÆõû?…]§½þ‡~?mzáwµ?Ó&Ù,g%Ò?¹½'ÒÛ
`?æÊÔrù?º-`ñNg3FGL J1045.7-2926@q	ÜÆø@9îσ³~À9:kÕ;0XÀ;"'»0?â"Åù/<•@œÈÿåí@¥bYât¿æ(Bn1y¿åÍa1É%οä+RÉGÿj¿ïÿÒ1ª`ÖAGNfsrq?ïù¶m Ú­?KýpqüœÏ?7âlŒùqä?6­•†?:j*l1¤?FìHŠî?ïΐE£Iä?wýkLõê?db|aöò_?gðƒ;Œ‰?m
=ú¿*ô?pãx'?ïT ·4|?Š…|mÿH?Œýly?¾:?5–sü¡å?Œm‹Xó#3?€&
Í'å?ïç?`Â
ƒ?ncû ?.Úé4YÄ?:°%k0Ĉ?fÒð¦5Ò?m¥¼ÌDçS3FGL J1046.9-2531@pèÙ'ÿ@=gqß@lØÀ:'8§ç:6À;ÉÙ³eº?ÌW'2_@cü3?ýŠ¿_&?궾ä½ëo¿â]'ÿ´'Ô¿Ä'ÿz㺿¿æJ£Ÿ#h²AGNbll?ïâ¶$Ã3?l	à<º§?RÅ(_Òê"?X £‰v?cçGýVo?fÛ×]Ã09?ïJÀçu?™Pê¢w!9?JŒc!þ?ŒuA˜Ì2c?‹#O9Ü	?nÑzABM?î½3	Ô÷??›ËF튶?
ø€GÎ"?ƒÐÎP¤?˜N¦EIÂ?…½'[8"#?íTçcû²B?§šTÈ'~?ˆ@¡)q?†5c¯×	I?²V|̈¸?¦ ߀6t3FGL J1047.6+7240@`׆@ €@DÀ¾ß¤?æÀ9ž.§³7ÐÀ;²Ä§d]x¿ôêeI/ôº@òfsÒ_´@mŽo¿ã~¢zòB0¿á币Õò¿à—í+ð|¿à*'ßB	AGNbll?ïü#W×¾í?>ˆt«ë^r?A^'Z}Ä?ÞaÀõÖé?9Té¡qö¦?</€–Mù¢?ïҽʾƒó?|™µ×w^Ø?bÌ
}°e?jý&QÓÜ?jv*Ãì]v?uf(§
Œ¬?q_È?{Ȍáen?rŽ5Ãf?gWiu—ê½?"\›,?v(ëG+Å?ïãJ¼ÝˆÍ?k|a!'Û>ü•F½Æ&?ÀXœ"Þ?l|éµA?jð-äOf,3FGL J1047.8-6216@r"ŸºEÀ9µ ÝDÀ8-r)HÀ: †ˆDÝ?öoôǽ™S@í/çú$Ê@<|z¿ãðÒ
¾¿èøò;‹
N¿èrz_'éå¿å3ø·P'¤AGNbcu?ë¢.VQF?¾†È'	/?še9-XŒä?¡O|àÐ%‡?¼U?«é?¼"KVÀšÖ?Ê©ûÿµWÑ?Îhf¹¾?Åur'Ÿá
?Ä\»øÚ[Q?ãø$[j±Ê?ÎöñÈ¿?äêìÕºøº?¶^óiÙ?½i'ëÏ?¦òªÀ×)?͟Ä'€'0?±‡G1gËv?á	05k>?¹/úRd¶?ºTÏ^?Ê>?²Š>xÈLŒ?×Xk¾g6ó?¹,,&+Á3FGL J1048.2-5832@qöíÿ'+¿?⏣?Ïg¡À6Sà_PÈoÀ:ü¨\ªü@.¥5¯v@%¼`CÃ@¢ùš
WÈ¿Ô¸…Jµ¹¿á_6›L¿æs7ò#=¿ì8w{ó§"PSRPSR?$YëŠÍ¬? !tœï"$?ïOä­#í¤?œ}õ=9²?•Ú¶"l°!?œqìµÿÊÊ?0á‰âíëR?S|͒ÒO9?íÏ6ŽÍ¢v?«©i-Ë©?±uiÿ¯þm?«½ºdGÒ5?qÍAêƊ
?gÜ`Á¤?ínŽiÅ°?¢(>=n d?¶·niÛ?¡ÂcÝ\°.?B'ªþøfp?C³^þ–?îU‹¥?šÜÜ`7É?ªd0£ùÎ?š‹âuÝP¦3FGL J1048.4+7144@`íßý`é@E#,?ùëÀ8ªE¹GµÀ;jä'Ë÷»?ð"……æ^n@hðÎ3Õ@"m`*¸¿âp4؜0D¿å·oK
¿è'µ"9¿æ€¾;x.AGNFSRQ?ïèp\G)?bš0ÿÜ>?b†öÔ?`9¹aî?Eôsó'ð/?Cu­tQ]Þ?ïOFÌGBu?"GN'âö6?Š'h?‹Um¬®–?'&0éœúa?'ÿòht'?îÜ.'Q?"k¬
"Æ?)³MV¯%?‰Â^'ùõ?"Pzh…À²?ˆbñ'þ
Ò?í­ëÎY1?ªƒr•íu^?œ7¹&€k?™&1r=ræ?§f‡,¹L?§­Sû¸h3FGL J1048.6+2338@j¦ôÿ†]}@O/ »èÀ9¹i,êCÖÀ;½WQ­D?ív½µhé4@?mÚÎî@Nvÿ»·|¿¥Ÿj7_¿çÏà0½ô(¿â͉:¦Äû¿íY¡ÃAGNbll?ê†Ê´Th?¾ó‹Io.ñ?Ã
ȺI?»æ£Æîé?£lrùѕh?¢v¹Ù¼8?éƓ()­?ÀîÈl%I?ÃY²x¾Ê?¾8üßí0?¦0›o:?£íª"2´
?èŠÍÁçñ?²Ô<‡]?ÈÚNeF?®°'Ÿõ?´—ã]&4[?Ÿ{€°#?ã°lY'k€?·gé£ãí?҃ PJ9?µÔÌ ì"?¸nõ›¿Á?­'Ï€åÎ3FGL J1049.8+1425@lÝ¿˜0ä@MË@ÒÎÀ9÷¿µ'À;˺µsô?Õ>vn3@Ëãæ™Òz@¨‰?"O[¿èÈ蘟¿ã€ßxöáÉ¿ã<æü+'³¿ïÿÏ7؀×AGNbcu?ïõƃ(mø?R¸"'7?E‰9éËè"?Geۀ2á?C\¹t|:Þ?E¶ëypñ?ïsÜÐùÃ?¤Ÿ"Fcv?"W˜Iv?…:eË÷."?}ÔèRä?µxÆBÂ-?î°õ…Mx?•>êºu?šo˜	ŽÑ?'¡¥cfƒ?ŽãnšˆÜÇ?¸šªëê?îéÙÝ<æ?'P À´j?Ž`;ð0Xc?‡ò·f-?""Ál@6÷?‰¹P.–ðr3FGL J1051.4+3941@fMp€0<@OjÀh:|À:s0V	!À;¸Ir9Ù@?Þxš¼ü˜@
—ÉøÜö?ú¡I …[Ÿ¿ïÿëü¨:?ïýøÞp¿ܮ'@òʟ¿x¶0d]ÿAGNbll?ï⢤ýb?gfb
\{÷?X%¨8>?WÜx¾…?aJ‡E¡Uõ?`Vµ«*G?ï¼6þið{?¿àðü=Z?q-ƒî†Ð?x¥wWe›ø?p¶ü܁¨(?s¤B'5Ú?ï)~–(á"?…ßìÝ+C?†`;næ?{Я@œB§?ž@Œ,Q?z¥	'³ø2?ï]ó!²¬?'"Ó«è­á?‰|Iê	ús?,PÎ>[?~
ÛR–›?€Î•W—:03FGL J1051.5-6517@r-'Ÿì™òÀÐ3³À8ҙ!¤•vÀ:ñÅÒ݈¿¨~".xðI@û)/y?@Äb¦-¿åÜ©ì£ö¿ëú¬{ôm%¿âúðcLM¿àš_ð´AGNbcu?å~7\§UL?əƒqa/E?t‹õÕ?qÓ©AܨA?Ô¯×%'?ɘ—F'æ?é)SÏÁÊ?ÆK5™Ï1€?ž¦BPåy@?¢Zå"Ùæ?Ƕ'f¤I²?Ã:6öQõ@?䐺í˜?ºƒϹà?®´ÏG'S?–á'7*Â?ÔZ°û4…?¸¶×ÇM«Î?çϾpkú±?°PÊdÜ?so¼ä`òÓ?qY€7O'–?ÐÄ+–†Ò?°ƒ£
ÛÕ3FGL J1051.8+0105@oD  ô×®@I¢¹¿©Î›À:(48ñÀ;¾º•"<¿ôÉ&úë™@¾g'‰«@…n€;N¶?à<LCûWz¿èuzýŽP¿Ñ蛡¿ãÙÝu«A§AGNbll?ïâØì=¥ì?q—k³€?;P?žª~?CÄçÕ?iÆIºf>^?p…ÿº~?ï¯{êLTë?†ÙÊ[%3?us4~¡b?¶;7Ù9?rÎÖ[4'Î?wGiKã?îå)¹ôP?‰*ƜÉ*?…yáA»—?t¾òW+¹?˜ß} ˜U?"xÕöžX?îÔÍ O¡<?™Ï
Ҟs^?JÂSzk"?S¥Îô¨[?¢H$­–€?™j‡ã`[3FGL J1052.8-3741@qf[@-¹@3uÑÀQ"GÀ:Aµˆ©\À;¼óË>WT¿ûrßsB—Õ@ˆnÙ§{¯?ÿðŠß—¹¿êք4ò>æ¿áž0I@]5¿Ò0¡Ðl6¿Õ-îƒ^wAGNbcu?ïüŽ3ÈEÊ?A-ìÐ;? ~[ëªõB?0)0'áè?3O3Çü(z?@+D>»Ræ?ï©aižàÇ?™RŒ\-—?d>À`o?k™Ø­?€˜$è/ÇÀ?˜è­ç‰,?ïSÕÀ"Á?¸x¹U¶?zò'DŽ<e?gçàmŽSú?'G8ô1\?z[`›&Àë?ïºé†ËU?v"ô{CQ>÷3®dã´?H¼(3'?:%G¹{?vÀ×¥¬3FGL J1053.7+4929@d*à~Zy@MŸä6vÀ9­µ|N/8À;'
ãˆÐôÀ .s±@mwô-cæ?ü»È€aå"¿èˆÂ¬bt¿Ð¹9#¯¿Õ,¯Æ¯¿á}"ð+2AGNbll?ïïeïZ¤x?žÔV µû?S{'…¼Ó?"A²<[?Kq hb¥Í?‡¦†_À.°?ïÓäC$õN?w" Ü´?bΫ )"v?i"<à=`?iM:ፁ?nÄUýÑÔO?ïFgµÈ¾ì?‹Ù$÷Î^?ÙæŸ"¾?'¾+X§€B?ŒŒ+î´±?ƒrI*ª£¢?ïß.ºv8:?nòWÁÅt">ñ'Ï{Œ?ÐBÍOK?pWC˦?nàê¦gF3FGL J1054.5+2210@k!«`kz¢@O‡@`B_÷À8ÕE!r@À;'°Ql^¿òž"•P‰°@¸'uåµQ@šþ¢Lœ¿äÒÒË?¿ä M¼¿âJˆÝ½=–¿à]Åsù2BAGNbll?ïù›eƒÓ?JRCò³ò¼? 얧 ?ð"*–w?G–lÀ,ϱ?H€
~Û?ïÒ­g4î?w܋_ÌÉ¿?bŒ¦ºëÉþ?hÂE¹Ç«?jÅòHÂ?q/¤ÔJOI?ïJ5¡ýD?""NyÏüÄ?xfTZŸðŸ?p2íEù½Ú?Ÿ¶©·»=?€êB<Vq?ï®cÓ:1?€¨)‰Iä?0½®üaœu?Hé$¡àª?ƒáQNfô?€s†î"¢q3FGL J1055.8-6025@r*@ºˆ¿æ°ÿðCRÀ8>öJt˜XÀ:0ÞÿÕ7Õ?ÿ¸VÉ}÷@μlØE|?ø¥ˆX‹¿êYÆO°‰¿Ç;šNº"¿å8BhҞÀ¿íú±°=PSRPSR?J™#â?Q>'ò»fm?íØދ_˜7?¿Ípø?V?±å"Ðöˆ?¿5ø?Gfl¢m?`[{¶/?ÞO?Ìz¨spÌd?àқ`v?̂é+P"?¤ñõ{%:?˜^á¤ÝÓ?ä¹ð€Ãk?µãœ=½"?ÓíàO$c?´|ñ$ùqÎ?¥^bÔÍސ?¡D{Á"¾è?á
xed
E?Âþ'me?Û9Bڞ)¢?ê}9ü$3FGL J1057.3-2341@pý8€®@@…ߨq¤À9ܕyyh¢À;·ûêlj—?ôgë†Ì7|@Âó5AU`@ˆàdõ"¿Í¹fb#zr¿ÙŸ
¦¿í~×?'ÄP¿Þ;Ê®d'AGNfsrq?é;¶¼ò?ȱ'ŠÒ‰t?Ê~ç"ñPN?ȱf'Ž¤?…B™®xk?Ž"! ž?ï	õÐ;ê?¢½¿l%?'¾Uê?™ŽeVJ=i?Šàåç?^Ö@Îó¢?èn?ƒzhÁ?°	VŸÑ?Å|´)Ü5?¬˦
m?±"›tOË?Ÿ=®ã…?é¦yÚ£ž?À {¨ú?Ã;¨t˜»?À(4Íùk?¨«åÀƒc;?¥‰ T­Î3FGL J1057.6-2754@q$±Ào@<{Ÿ³À:w•¤A"HÀ;ÌPwؕ¿ãÍç˜ÄÌ@{f°6?þ,TßÖ>æ?èvK6gΤ¿ã%ZºÇοß@‡ë­sҿ̎)‡ý~µAGNbll?ïêøÀßÒ?d6c›Î©ç?AþнáT#?E€4Œ;™B?`‡Šðµ™{?a˜ÛŸ`É?ïǯZ?NÄ¡|V?g©k"Ti?oî‹}R
?pSoÀÏ¡?vH2Cú?ïRmø!±?ˆŒ¸ºSz?ˆå í£\T?}kç=-?'ÂáÊ*¼?~Öçµ'?ï‰jß·²?…7fDrQ?4ËQ¨tbŒ?;"V+∵?Œÿ:Îp1?…f®'Õˆ3FGL J1057.9-5227@qßÔ§e4@"àà*!½À5öU/}ÉÀ:—«bï¹a@JÝð
¿w@nFM—7•?ü,y¦Žu¿¸Ú§MXŶ¿ÜáåÂUê1¿éL)õØðÙ¿ï¥Ó–7óPSRPSR?0ÞÛ¤)y®?5"æ"Œ?ï»ÞìËN?"Iïê¼%þ?€´'g«à?"2X‰-–?4÷Î)û?VŒÜ´ÝËú?î¾Q-ž&Š?­1¶…Óv?£ñí6Co?­3uˆ"<?Šáç2Ka?ŠÓ0m!ÏK?ëיÁ
K?¦ÍxÙ]%?½æõÕä9?¥µIn[+>®'YúëÅ>¿Ùû\$â?ïûˆyYÊ?LC'«Á¼"?Aº9"/?L;ˆ5>Ú/3FGL J1058.1+7010@`ûrà\̊@EÿüŸù/+À9vëg†ùÀ;à±û.·¿ã§|p¾Ùð@Cٗá]¨@ŸÜ TsË¿æçˆûÅ;g¿éO>	X¢¿êùNñˆKœ¿äÆMy'AGNfsrq?ïõðñîz?S,lÉpO?F'%ÑßÚ?Hˉ(z?Aºuº÷Ç?FuEó!ñí?ï«ê®;Vç?ƒaÑ=Õù?t"¢…?{E?y1Ú»y׸?u†]@?wX?ïM—©cË'?ƒ[sê?~sÚFÑ|?wÏÆWSœ]?K[¹éÍÒ?}(ÐN
L?ÓjD?uŒµzË?aºÏÅf4œ?fU~Gû–?‹e—Gá?‹ëí³Ê3FGL J1058.4+8112@_ÿ+@öjU@AdË@ÒÎÀ9…Aî·Ù À;u¾¹å?Ù!Ââ,[@NiÔÚã;@T3‰M¿éò«ð"7¿æW˝;©h¿ëx`!ÿêYþQæ7éAGNfsrq?ïúï4N7]?CÒªÙ CÜ??³Hé
QL?AM·¨ð
?!¦)Jobð?"
Àöë?ïÊj]úø@?wрwj;§?fÒÇ™Ï=?jWøéÇð?nÂÚëmïZ?q›ÞȄ/?ïB
r'—?"Ãf?,Þ?ƒýXe–D?}`+ƒæ	?‹€höø?{Æ1·Mï?ï`çJž5?"Ú Ïq]?\ƒlÕ/1À?_¸€3O?ˆWX'²Œ¯?ƒ‹³7ëÏ3FGL J1058.5+0133@opŒ€A@Jc*`%څÀ7s\#íEÀ:µ#I±#ú?òè³ÍøE÷@Ð>â¾ÑŒ@碥0üw¿àã ïá¿äoÒBW"¿ã•ýmt¿ââ0-¼ž#AGNBLL?ïøD3—*?Ph`^åè?,äF ×ù?2V°"f?G¶ûÎæF?Kk0•!®?ïÙ"Ua?u¿"ÂÆ:?cal.?l€žòϲ?c™Ø¦q'?gâæ²Ý^Ñ?/P?›ÃϨõ?Šê÷o;?‡w'7+‡›?žÌL ÔÌ?•äž,x0e?﷕•\ù?'·j\¹6¦?0)µà …&?>ÐËýr?™M	£½È?''O°rOG3FGL J1058.5-8003@rŸìºËCÀ2G?}ÄQÀ8%ðT'RÀ;*sMÕué?öfnSŤå@Õ	2®¨õ@óaDéi¿ÝÛ³'×hæ¿å¦,áÉ¿ä‰][û©Y¿çØH»/ÛAGNbll?ïÞ§E¦âC?j¯>Vz?T1R|ƒs?S²|/_ï ?g@MßzË?eKëèÎðÆ?©Ç¥?ˆœŒ8«A?bŒs!û·­?i©p¥÷M²?ƒr8ðÏ(î?"ñ*>'âl?à¸Ê?'»×Ùg"?¡!K22Ó?'	÷øV?›­ý^OÍE?ŒöÌãÒ­?ï	øõÆ.^?›?ü$Èùð?aÅ@UÕ;è?e\t'.u?œˆ9<Œ?š²…vP­3FGL J1058.6+5627@b³fàé´@K8€iFëÀ7é´[¼¿9À;2¥n¹òÀ  :G¤"@'6MïÍ?ÿ€y¿ß)²_§õ¿à½0o‰z¾¿à;QÈÕ¿¿×'m½@AGNBLL?ïüäó¥?3¢ÙÜ^ã£?	$Ðü´?	a+MÓI®?5µB¸])}?2î?¯R?ïÞº¬Í?sZžf?\·_N2M'?e)úKmB?bêD@:ú?j}¯*tÀg?ï[€ D÷¡?‰¯üÜÂe³?rÝ ¶pX?sb"–i
?±gífߙ?‡'9ýøl?ïïÌtŠŒ¬?e¯§
fòƒ>ÆjÈö£ÇÄ>è»<qíXc?`-ðÃ5ªl?e­qÝÌ¢3FGL J1059.2-1133@pšÑVŸ@EYá @è(À8AëÒK'À;4]"<?Þr!+û1@ÓrDëíN@qÀa¯r¿Þ¶šm¡e¿ã/ØñÚ^—¿Þ"]
]qÜ¿æîBøFAGNbll?ïø",¬d?HîÿÚ.æz?0GŒ®âõK?,u®¶ã?G"°õÜô ?E*ýoc¢ò?ïºjôü*?~ù	Ðñ®?qŸ¿^ŒA7?t'}ðË(?q+7&õ©÷?r`Ü+Ì?ïWŒ^Ô?†¼-3²Zq?wReJ»¦?p¾ˆÔ-«?ŽªBþ7æ?ƒx—"]w½?ïÛÒ&Ûg?—=TÌÒÆo?b"êaœÚ?dDŠU£g?œònñª?–ÂâîiÜ
3FGL J1059.9+2056@k'_ôö@Oî2à'¤À:kUž˜À;µÕЁ3?ê—×p¥ëž@gßbP­@Œh€Z¿éÌ,QÓÃr¿åÈãï(Ah¿î±}cX?é€4
AGNfsrq?ïóú‰¨â?`Ä>ÕS»?U$A›•+?^t™þӔÛ?3G'PJžA?:€{î– Ó?ïÆ.øÏ0@?þ¬ºÅÍ]?j½•'áð¥?y†2Ñdž:?oqžíÎÌ?s/ÌS¢–?îÙ-ÔëÚ?-p孚?'ìZIo­?†œu
íƒ?'ñßûòז?''ÏDÝö^?ïʞá&û?¥Qùhü°?RŠûÀ^¦˜?màG"w,?v
Ð|äXê?'õ±¬¶–3FGL J1100.5+4020@eù«ÀãŠ~@OÌÚ`3F~À:
µÙk@ÁÀ;¹u.€F¿ê_hè™(@µù÷}?ý]À?u¶»?ïI¡¦¥¾
¿çÐ2ÈTB"¿áZœr€À?ÇàE²^.AGNbll?ïõ'hÜ?T‡¢¤ Í?$m</Â9!?)Ÿ"÷_¯?RNy6å?SL=(I ç?ïÛÑFªÁ}?tsù«€×¤?[¶4›W?c´¿
¢u?fS²O$4Ó?l©²ñ€Ía?ï¾~qG?ˆâë­¥¥?ƒg»X¶eÑ?yb"I?'ô_ÃÖ¤Q?"VŽd™õ?ïÏntöI2?~p/†)I?W‰¥‰?Ý_*«i?x"¼ÕȈ?~X¼Td3FGL J1101.5+4106@eÁŠŸb0@O½ÿôA†À:U€[À;Ð>åE¿ø¾"y@JDâˆõ?üK_¯+¿ésã@pw¿ÀƬ†J N¿Ûï kfg¿»|,êLmAGNbll?ïüÚo+?4 T‡S·¸?$×ÿ8‡Gç?%³5I%1#?-dǺý?,X>i"i¥?ïÕށ©?xÀeŽð?bÞS£ n?iP;M¹,î?h͙Ýéq?p'€¢² ?ï׋%¡?wœ@ٛ¿Š?x)3VøÀ?mØ;A"_6?€¤ðqº7É?o07jœS?ïòðFŠ?V•á4içL>ð,zWÅ~¾>ýAk1\V?Z¡>6Ó:?V{Ò"é3FGL J1101.9-6053@r ¿p¿é±}À9rÀ7Õ8[' NÀ9Ò%çñ?ý'¤ö!d@	1‡úŠË @	¢®@D¿?â̤žZs"¿àW6³t ¿è…ÂÖ[¿íUç}¨!rOTHERspp?zsÝZ&Î?Ba*­†?ïoï§?§d¿òÃ?ŸC·Ž-µÝ?§_Œ%;>ú†D}Ñã¹?&0FH±ùx?íPi([?´çBuûÔG?µ}\Sà?´ç5™;Ê"?'òè,½ØR?v,o¤L?èû|-'8?µñÊŵ2?ΔãŒ~›?µƒcçEé?AÆo&©"?C;˜•õ?ê(;G"»?¾ž²g)=?ÇMM;»ð?¾›;Øm¤Æ3FGL J1103.1+1155@mÐ~KZ@N4_²?À9œ''%àÀ;Àæ"ß(¿÷ÒL%r€P@Eõa™š@#²`dä	vW0y¬¿çàVqH9!¿éFûzgص¿Üê¦+ù-(AGNfsrq?ïý4d¾Ÿ?3¨üNY@—?÷åÓc? ñv6†û†?,¾<$#?-^—øGÃ?ïØ`l»
?vX*"ÁUŠ?aRÓQõ2ù?i(]Dµw?fL¿òýµò?mâOrÍX?ïpS­ÃØÇ?|}íºüÜ?vù¿GÔ|?m…í˜ô#?ˆé¯eä)?w]Ò°Oòí?ïüÃz‰$?BtKÃ	6ï>ÀÛyäŽ>ÙM=x\|?9Âxð{?Bn1—ý3FGL J1103.5-2329@q×®6	@@‰¿¿ž!À9á¢çrÀ;lelkc%¿ì¼A/±Y»@Èvç'÷?úPúa¤¶?ïõz?ƒš÷¿ãx39W(u¿Ø;âŒÛ"Ù¿¶y‰âJAGNbll?ïÝ­]Ž}?ue!8Í?BˆýλG?I±+èKÒ?m°bþ7±4?sàâóƒm?ïЊj?u`×ä›ÏŒ?cÑƳgá?f_m£3?k¤Í.T"?n}J¯À¢?îi,ßy¼?"/£"—?Ã»"Ö¡?è%¥¯ý?¡T}]`û?ŽÚSæ'u?î²ãä¦}¿?šG‰KpEQ?+é·M	F˜?6$±ûT?¤µ×þK»?š@1HÙB3FGL J1103.9-5357@qöÌÈó#@—Þ_ò.À7ø_ð*ŸçÀ:׀·J"‰?óˆg¢Ñ{³@Ö[uòu@$6ým(¢¿àOéÜÊh;¿âý#6pY¿ã£¨™ÅA¿äfÈ\¶ËjAGNbll?ïgß_[l?'Ž0²Þ?Hvb,i"ö?Jß%ô°~?'@a<	i?'FUæÂq«?î(²KA'ß?±"Ölv?s­eò>r?yH*¤?¬?ªÿ.«Ï:G?°ÔH}y€?ìô¬‰y.E?£¬ìèjƒˆ?™†' ©"{?Œ½dpXn?±øûE4? ¹í¢Ÿ.?팤µÙqF? ÚæsFq²?uËuJæ?w
†dÈɞ?²>"ø/Ço? ›ÓÕ§$Ë3FGL J1104.3+0730@nµ‹¿PãG@Lõµ ÝDÀ9'UM9oÀ;­`˜ÇÃ?¡¹‡YQà/@ÖR²o@‹s'ÿÝñ»+5q¿æe ó$¿ã'åcË,¿Ù(•M¸"NAGNbll?ïñ+۔ܺ?b®tO[?6ô'Ö¾†?5r:?Ȭ?X%KÌPۏ?aFqŞ?ïÅwtŒ™?}Ø!Œg?lpñÙ Jã?s|+¾B?n™šF˜"?q¹>"Û?ïOD=¬{Æ?…ó§Mn2?}¬°µñ+"?r¬¤Ã?X˜9èx"?€[tôßA?ïV'ÄÜ¥ª??´òH›?ZÈEé#Ì?aß×L¾²?"ŽƒÙÎ?Žï}º23FGL J1104.4+3812@fzv@c^@PB7¿õMõÀ5®à×E̓À9²‹-Æè¿àµƒíñF@æbu+?üX¥€'œR¿×Dû]õ¿Ýn(#¤¿×ÌæäŒBT¿ÔZ½#AGNBLL?ë'%s‰ßÐ?ÀÐrþ‹?W[œÐM"Ù?mÁՐ¿âY?ÁȲø7å›?ÀÄ7×<fò?ïØ4uIÔ?zA×#˜?]Õ¸O ñ?eëՐ/;ê?hà®Ó%³+?tþÆw™3?èIIÀ£@?²0"7YÓ?"fœ{6Ü?"ï4ݯB?ÌN	ã–â?±¹ÞaÁØ?ïÀ!¹,?‰hUw¥kÍ>ÀÁŽä)Ô>Øfs^´Ï?ó×MÆæ,?‰h
‰²tB3FGL J1105.2-6113@r(ßÒc¿îðÉ'ÀÀ7å8ÇǪÀ:)óð?âö''ž!á@7Ý¢@v;Ÿ"X¸¿äƒAy$·£¿èbz–ý˜¿ííÃ3é3¿ÖÜßb]áPSRPSR?NåþŶ??œëF°^?µ³/Wvž?¾ ®Ù•o~?ì_"å&£z?Àvh	à,B?¸0åQ|è?Áið¦¤?¯¦4ï1²•?¶Ô°ØHPÙ?ëö"bµ9?Å>âڐ^s?¼RËÂ×#¢?¦‰U""x?ȾÚw?»?±òĪ×B£?æp¶ÑK?´ÈõzÌ?ÑÉPPÀ™,?ÁTª3·?‰¢
ÊT±°?Ç/HÂ?æ´Ï v`£?Á"Pû‡¸ú3FGL J1105.9+2814@i¢ß"xî@P«à"'À9¾‡«ÚÀ;Á¹žòžî¿Úãå¹þ@¹F–<lî@¼¾@Bo¿ç7âR1Œ¿ã_¾«e¸°¿ç½®J;ô‰¿é—ùUŽIQAGNfsrq?ïòï‰Ý›B?[$|5©?Qâq4*?Wå¦>R¢?@|¹§*ëÌ?EñÓ9-X?ïÔLe>—<?xy¬ ‹?bà8û<î?oi`K8œ?hÓaÆ+Õí?p>"5ݐ?îô?oJžg?¢2£ók3?‹þ…ÓÍWi?…Ž_ÿRߢ?"xÏ,Ňt?…ؼPKË?ïÞ	m-'R?s½êÒ Wø?A`¯r&v?LS½õ9H?mžŒ&'"t?r…^ì3FGL J1106.4-3643@qˆvŸÏ=À@5‡Fÿ˜ÑóÀ9e‹rXÀ;¡6Ç<j¿òñî»ÚŒ@‹U@¤4þ@V)«0ñ¿äÈé˜+ý¬¿äþÍGñÜ&¿×ä&íÌîþ¿ì1 x½ÎOAGNbcu?ïˆ"—'1%?ˆÀ'¯Ô?ª:AÜ?€u9Ù»ª ?yã`ré²?}4^µ¾?ïŠýx?—Tÿªe?v¡ÚBkª?{ŽÙð'Î?ï«w™ì?ˆ'	Ûúv>?í'DÍɨ?¡–U«lÔ?§‰gfwÐ?š:¾uÖX<?žÊè™X•–?é®¬g§x?ï@¹	.}l?uØUv?M]Éé‹Ö?TÔDšðeÊ?–ýð'1V?.åÏ>3FGL J1107.4-4447@qÃN?þó'@,‰9¡}ãÀ8ÉÔCédÀ;bŠ÷??åÕè K‹@…B(o@¶@ @&¿åݚ?½¿êõ†ÿ'å¿âK>}ý¿ïÿÛ*f8¢AGNfsrq?ïñWŠáÖ?‡X.¶3Ÿ¦? 9`í?Æ$½Hz?[É_–U&¡?‡UbðRVš?ï#ð
)(Ý?žÞåèÓú?|OfÈÃî"?~ŠÝ¢ÀÓ¸?"n$¨©èÏ?šœúlŽ?î[
PŠ.é?–s"ÕÄ;?•éU'ØÎ?‰Çïˆ?žµ`o(J?öµœÈ´?îž;Æê8?Nvc¦ÿ?|nb'ŠÔó?üÈÌύå?¢'Ïñ`ü?›V+Õá^ä3FGL J1107.5+0223@o«àe0@Kv 8ðÀ:(¯K²†À;´p'I¿Ë";ϗŠÿ@tRY«î@¿à߃ü¬ìæ¿åá̧ý¤¿çN±Š"±¿¼
-Ux­fAGNbll?ïÉ#oxò?›kHUÜGë?`yÝ28?oò$¾èa?s1¯=ë
?—ìVÇÄ\?ïÊ¿-Ž É?{g"ÕC—?j>¡a"?rCémo³?k¹Ïý©?op[G­¡?ïïf˜?Ø_¬]ïÔ?‡š'÷hO¨?€	/½Û"?"ryxԃ?"üx¡V?ï"͆Uœ]?…¦#ïØöG?E!ŸƒÝ÷?QR6¹3?‰º"rgzž?…nù'‹"Ù3FGL J1107.8+1502@mIÎ ‰ãC@Oˆa .QÀ9®JGKîìÀ;«å3Ëßg?ч–u*'@"þ¾·`T?ÿÙGŸP覿á
/±|¿àVY/"Þ¿Ó‡Twüeí¿äþw}¶^AGNbll?ï̯ôæ¾ñ?tº³R`–?`,̨qx?\•õ'?q'Ÿ8XO?pÆÕºÁú?ïbèx?Ž¼>aùòy?"Ú™¿ž2N?ƒ•§>n?',>ƒÉ9?ƒ<#?ïà»Fk?ˆäޜԁ?"¦ÞŠ2‡?x3±^› ?"yYÝï?Ëà&¦Ç?îX#þbV5?—"š<SÛ?‡µ%(ŽU?€(ŸÊœÖì?¤~y1?•aþô°ÿ3FGL J1109.4+2411@jÏu@‰]@P·þ¿ù³À:\ø³¥À;ՎñŸêì¿ëœMÑD*Ò@
œ¯ê"Ý?þ0§á6¼?ÏQ–íå¿æŒâaÖ׿ßÐïì·xÓ¿ ­Ð¬*AGNbll?ïàBM#Æ?rx?"è|?;$õŸà
$?;°—|K{?lY(@y>?q¢5/œ¯…?ïӑ2*>é?yµ®+1!?bÓ
'k…?pTøDŒ4°?i›ÀDU'ø?p<8"®ë?îèÔZª?‰"¯^M5"?ˆˆgí'Ã?xT²zj;Œ?–¡pü)VÕ?'\H²4?ïľ6\ºˆ?zVqÚFE??¾IHÙ?1ih ÐÈ?}/å×a—?zF–¡"m3FGL J1109.4-4815@qß%¿­)™@&r¬azŠÀ9¥—­[îÀ;z÷Zï:?æbÈ
í Ï@_Kä/@ôÖ ˆ‹ª¿ç8äl?ˆ¿æuºIðí¿ég#™Ñ烿çÌñZAGNbcu?íې•¾?±¸"j\­?¤ L,Rú´?ª1lQL…?œ[u"¸"?¢,íá#?èǑڶC¶?ÈÀ¥*Áýk?¶†B…'^¦?¹ÐfQp¤$?Áž—R]ÁÑ?Á`‡ì\Ú?ìB7páý?¤Ýøàr?¢é–îØ¢D?'+|ŖC?´y{Åžö? œ§'¹œE?ä«BìoÂW?µN‡Êa—?Ä÷mº?´ŒEâ?É<üá$õê?¯òèîG½É3FGL J1109.6+3734@fµ'Ì÷@P>àŸ°À:ٟâˆö´À;íܜM©?ىƒ•þ@
ËØ:&—?ú^Çá?â
¶?äê?ïø̜§h¿ÌŽCE鳿̸@	¹ŒAGNbll?ïíóÇv/‡?d[8X'¸w?Qè?82g€?WÈÓÙáÚ?R01Ûn†ƒ?\û]œ€h?ïsìÙA_2?'"y­vsý?"VžF±h?‡üâ÷.?}Îæ"Ã}?'©{¦ATi?îÂÞ§ŒÕ?'"6ºé|?'­u684?‡úJR"?"ö¶
ø-B?"ã]¡uÇ?íšXGÒ0?¯Áv.í?¯ZݧO?®¦´ÏAŠ?‹þ†_n8#?ª$,€3FGL J1110.0+7134@`µJ`"@E°…ߨq¤À:P­'tâ*À<î
46h?â¸D{"@ƒ`ݐio@>îÿ|¢h¿ã5~VƒV¿ä¿ß"ƒ7á¿Ñú,›-\¿äDŠã76AGNbll?ïÑ·¯7™ð?x¡`»C"?[˜¾™¢¾3?d374A¥?p=ø½ÊWÄ?ql>ÀŽf?ïJ<¶	#?˜`ï«°ÁÎ?'½!u&'n?"çªÜêb÷?‡3-è0'Ž?†=îœõ?îò‡ßˆ è?']×b¢5?ŽËa‹ÖhJ?‰T™ØU?'ISI®á?'Rk"i…å?îõÜ¥yÉ*?–exǎ4ÿ?'øAü¢9?"P0]Kj:?—ÈJRu½õ?'hú™¡3FGL J1110.4-1835@q6_Ø­¬@CȾâ(À9Pc¥ÁÆ	À;uéÀ"š_?å'ÎÕÌ@x^áaÚ@)? ~æ?žÞ¤Kàdj¿ãzuNX¿Þ¦¤*Ru)¿Þ÷Aö¢>AGNbll?ïÄ<Í3?yAR¦n?iå6ÒãJë?kÄ}ÐÇì¢?pîþ@–?r<‡ô/ºÙ?ïr˂
ô?‹Á$"+"œ?ƒa8™@:¥?'^rfˆ*?×ÍÆñF?)%.
M?îͺº?'VäIOL]?P_1\[?"ÔMÍô?– y$¸?‡åqe±¡?ìÖK½cë?£|ã'œ?ÿ©Bè%?‰Æ×êŸP?µ
·Ãsfª?¢°e†À&3FGL J1111.9-6058@r2iŸ¡—¿Ù<ޟªw/À7æ>)0zòÀ9ôúWI'ñ?ú…aêhi@0{âN"8?ü}¶¬¤ä&?ïÿ‡¨3¿áÈ%Qâ傿å<"Qw°ª¿êý~ñL³ãPSRPSR?‰D	ø٘e?ž/ê`Ó3¼?ÀöUL™b?››–¯­?ë]Z"öA?ÃWjÇÒã·?x•Ìíp?'­Pc`Î?¹œþ@Q6ü?¸þ'G|ÑÐ?ì›66[þ ?º)e¤‡Ó?¤Ež:Íô?˜
{ëq/¥?Ñ‡ç­í?¶1J}³?æ-ŸØ_IÊ?·øÂüp¬?¬ÄÌÑiQ#?¥{­S4Þ?Äæ	wà2v?´â9îu£?èú0Ôñ^P?¸ÓjÏœj3FGL J1111.9-6038@r0Žàm"¿¶nŸËùÀ74éœlÀ:Í<^U @Veòùg@¿lÛËmQ?û'ýXZßõ¿àÍD@÷–û¿àŸ|Ò¹uØ¿ã@Pó7š¡¿èŒZ{v™OTHERspp?YtI áû?WS齜á?ÎϏYß\Ý?ɸcÇÑñ?è?b¹˜W?ÉÄXœ°Qª?1ß,X>Ãi?I9O÷ˆ­‰?ßQ0Sj°?Ée -Âé?àU+ð¿ ?É¢Ð<Â?¬9Ÿ¢$»?˜Dãm	íY?ҘUÇ	zß?µ¢w²»Õš?äð8ò E?¶Œ`)ñ"?ˆ)f?'Btžó!‰?߬0Ý¡?½6#Dü¿_?ߓFüEå4?½˜f•ý÷3FGL J1112.4+3449@gZã`'@Pàg@™ÅÀ8ðùÏ5]À;­Ôèë?ôÉ5M¿¦t@v˜¼¤áv@Á»=iè¿Ü €±žÒ¿æ·¶Õê'À¿éÇRºb¿ç6–ŒkU0AGNfsrq?ïïA$ǁ?Y)k™@	M?S½Uô¢Ï?Q/ÅD£ó?Kßò6Ki?Kƒ}.›$?ï§ð¶5ïþ?‡â',Eí?u/:F/—?}ûiÞº™Ü?vØjžØõL?z¹o«š2Ž?î‡qzx•?˜aáÜ&~?—D ?°*?Ä$¾‡?—ͼ'—=2?ŒN,¥^\z?îφl^4?š¤kj9?'þS}Jó?£€¿~p?", ¼4Z?•÷í%cÀ3FGL J1112.6+1749@l¿VÀÖõE@PZßÎ1QÀ:×ï¤h)µÀ;Òÿ¬óéq?âº_ð*Ÿç@ó×QÑ?÷x‰ ¥'õ¿í-?ö‡~¿àåñ!ö¿Í`E|®HË¿³"‹RYBAGNbll?ïîOeÞì´?aTªÚ"?J́å6^ÿ?PÁTœ¨C(?UúóO‹iÞ?[2Pe&?ï»ã	¾&?ƒ²i˜¿Á?pbVðàgÌ?y°ýtÙ?q¬$0«?t!¥LìNà?îÿg¯ç_D?'FxB†Ñ?'¹fX›?ÿ)¾êÙ?Œ³GUêøÇ?z–ŒmnÚ«?ïM¡ó'A?¢¬À؎Ñ?dòßbö|¦?u7–ÞÇ¿?"¯ïÕ/G?`Ķ?è3FGL J1117.0+2014@l2؈v\@P×°`À8œnØû¯8À;"pdìêÀi·|¯Þ@=oxˆÒÍ?ýÝÎg¿Ø£f^P9Ì¿Ý,éo<EM¿Û•7	V•ä¿ÚžoP^«÷AGNbll?ïþkLêOè?*1Ã-ÏFS?ã6ËÊ]ë?ø|4¥	¼?#c¨ØS?(Ôë'{ê?ïÚû53«9?wœk¯´}0?Z1LŸÉÊ?czVÑ?gì$|p:›?r°¨·ˆ°	?ï]'E¹ž!?…=¬þÙ9%?{ä![…o?y€‹I6—?ŠÄãÕÀR?­í|tLî?ïÛ¤æ+ÕK?uæë.èM2>â÷·¹`>ú6$Qqº?r$ˆn9Ò?uÞö©íEW3FGL J1117.3+2546@jgžÿŸ‡ð@Q:þßÙïËÀ:']æe$GÀ<
µùK°Ø¿ä…–À l@
]zž,@,Ù¿úVs¿é&•‹Bõ¿ÃÑ9æM¿å(©òçz¿êaÃ$#îAGNbll?ìeïâ]_º?¼"[•5?¹¬jƒû'?»AM2óæ©?‰ ³P4~?Ž=Qf?ïÒ­ˆóÛ?¢Ó*‡4ÊÝ?')¯n'G?½ÎQ'­‡?‰wõÀ yþ?'ÐËžŸ?ìmϵØÛ?¦ø×:Í[?²Û½åâZ?¡×¥ÀŸÊ®?¥ÿ˜Ö­?"®÷dñj?îƒÁÀéO¶?¢1èXâPƒ?ž()<##?ŸÛ\à½v¶?'_ž¦²ý÷?‰'nkoŠ3FGL J1117.7-4632@qéî@…+N@*¯a	/TÀ9…oîMPÀ;tÿ^Ë?õ{ât(ñ¼@ÁQ&
ZÜ@qA%iǿѱg
üx¿ë2ÉlCÉ¿è…î)qq¿ÖÏ,;OêØAGNfsrq?íh—c|³Á?´(@˜ZÖ?©ê¾/"1?«Ý0Dá? XŸ
0Æ?§¹?t(¾ú?î‡!ú-8?°OÚê‹À?‹~	ë½í?™Ã&ï—? ®]ä­±5?§ðNHS<?êÅÆ"mŒ—?ª"Xà)§?µæ Á/?¡øÚ~Èáí?³ë.+ƒ–?¡-øå²)?꺀:xÚ?µA·)óØ?©Â­£?®ã'<w¯?½Jþ#j[?°Îz^hé3FGL J1117.9+5355@b¦²_c<æ@MÑ?ùSÀ9ŠKn"['À;µ?Cä?èY²òÂ;
@¾Æ/ú™?þâà?Ee:¿ãTö0À´ˆ¿Û¹Ò;C}¿Ü|¸¦²Ì¿ÜdŽ="¨ÕAGNbll?ï±îÎç	r?ˆÌóš­ ?m 0Á'ª£?p¿<î|^?x8€+²që?éYt÷D¨?ïs)dùüÜ?Ž<ӏ…È?ƒ½øЇãÚ?…E¹ôûÓP?~ï[áñÉË?ŠéBø~?ï
¼Ç2Ã!?Š=~,ðP?ˆ(®TO­?|öyw'Úˆ?'"ïň?B¥å`…­?îL_µå	Ý?œH"ÚXªÞ?'´wüeë?'oCŠMû²?¡ßÈ£¦/2?–6rR3FGL J1118.2-0411@p{1\1@I·ª RÀ93_?*¸:À;ˆüàÎð?ò_9ßÞè@™+û[€"@…è j¿ã1Ró9j|¿é–žN¸ä¿è_x՘'!¿ïølD"@AGNagn?ïú´ôҒ3?@ÐËI+?5T&Õu?1ÕïÄq*í?4ÉNGŠ?80úëìA?ïÎÝVîã?{ö˜7h(?iyŒ-ÉËß?tŒM7‹zt?g©ãS//?lÒE®ç?6º3š?" k"p}?œÀ
¾M?Žg'ñc	i?'wù¨Î'?…s"|R?ïÏòhˆ5?€7J"Ü>?Uó'S»´?d_ō`(?rõBç&öå?{›©fn3FGL J1119.1-6127@rBTߋr¿áVnßå6À70ˆzdØÀ:I=tՔò?ꦥ3‰Lù@ŽzóXh@ßÆ´{G¿Ý"û10›÷¿å-æ‹Ý¿åÆFª0¿è–Ý
Bà6PSRPSR?Ãs2¬ÅÒ?À…æþ¦?¿â埀¨?ÀF¥Amˆ?ç&Ö Þ¤Ë?Ç­V{*ƒ?q•€_e
S?ƒB0mV"€?¾R0u?½…ã1‰V9?ì
¹A'D?¾	üƒ¼¿`?Âÿ¤E'k%?°ES¿¤¹5?ÅT&<LÐ?±o5MNõ…?åë
_ˆq6?·Ã5æþˎ?¿«sL¨D‡?¯82ˈÝz?Àöþfù–?²Ø¿þ?çÌÑü¬¶Š?¹ªp¡'¹3FGL J1119.7-3046@qŠA [À@<J€VÒuÀ:¼*JVegÀ;ÔËÔI¿×)»9t@"e²â?ü?ø¡, qúï?ÕQ{ˆ6šÇ¿è3Ñ\î1e?é
bh™¶9¿Ï€Œí¹¬_AGNbll?ïÏé1Syì?zs³¾R'?6Þf`6m"?8)s ž^&?v€ð?£[?zDšBy¬–?ïÅ_y(pú?Oïcu?g02èêÜ?s!tó¬?q¸)÷¸Õ?x£$!š?îÿ2" •´?ˆiŽ3;›?‡ ìaU'U?­ ³.B?"I9;Bˆ?€Ö_M¢'?ïŸöLá[?¿}aO">ö5NB¢o¥?®´VçÏù?ˆ2çŦWÂ?¾…ýU3FGL J1120.8+4212@dúë__(@PŠ¿Ý/ñÀ8Ç¿ÝÑÀ;øãú?ÖNL¿ g@ÿyZ3þ	?ùܒÉ仿â_qü¶cC¿Ôô¬'Ýóï¿ÎÃÕÍ|u¿ÇG¶Üå7—AGNbll?î,ðT&ú6?°;Á6"ú?yŒ98Zc?€Q«ÔFÂÿ?©ÿs–Ž1_?¯}').?ï•'£ÃԎ?‰»ÝÔíˆÄ?y+´Á@ç
?ŠeÁ)-K?|@y\ÔÒ#?€u6$"'"?ëÁ¤ÒÙé?¦N‹jx™¢?¢œÖýIÎÛ?"Òž­¿ç¢?¸¤mðÌIK?¢¹34I¡ù?ëN
ë÷?®Çáy›,Í?†	®Oe?k¹"Nù?Áf¦õn^Â?­˜n7y3FGL J1121.4-0554@p£Â # –@I9PßìdBÀ8H]®îÀ;NO~ÃT~?ñ¶O)Þ˨@ÌápGæŸ@î"ßu›ã¿à±`²iÁ‡¿æ'þ'o¿ãÀ¥«ºrF¿ìd{йtAGNfsrq?ïàð+($?fŸ=ÕDp?fÙ­TMÒ2?cìæÈ3¼?PlO\Í?M`Hïñ†B?ïÑß2s¦?}çÈì˜\‰?f¥ÀùÉ©?vPtʑ?g{'X¦?q]÷"õ?íékžU¢x?œ¶´#¼•Ã?¥Úò`_j?–«7óZý?˜ÈÖPŠò?ŠªÓÏ$?ïññKŒ!=?d=­
ȶ?'¯)è?@Sq-?Z%=ï͂®?cš0æøm(3FGL J1123.2-6415@rX'ßüTzÀA¯ó£À8\š1o
ÕÀ:áN_¤?ø&»˜Çâ'@g?A‰b?@å¿ÚËè÷¿ä[[¸ã`ã¿êŒ#0J_¿ëd—iò¸¿áHê¥êzAGNbcu?ï«Âvå3?"©é×``?`ꈎ†K?lMÊ*ž?€ÔÚ䏗?'>CRt-Ý?æ~\xß7º?Ñ^}QJ?¤
bm¼mÅ?°êUÙÅH?ЁúÀŠÑ?Ïðû2ë¡?ë¾+¥šzž?¨eÜmç	Ø?¤Å¶k]ji?–käìÌ+/?·«Ç}uÝ?¤ÀbØ^À•?îu$˜Cú?¥*Z*@R?t§"¢t?¢"plG+?­SÉb-@-?¥.Gël3FGL J1123.6+7231@`xÀ Ç@EˆßÊÖSÀ; ýŠúaÀ<*%@+i:?ñ_ &P¡®@	†ÁEA?ù~sÝ@
¿ì'‹'nŒƒ¿â ×@n¿á^ȓy'?Á.å»Ü´AGNbll?îö(Õú•?®6êaxù?œ.ZžÛáN?­³Ò¼~ì?t2*‡E÷Û?zp'ç¾'?ïMã`]Hg?¥‹lKý?ŠŽ{ -É?¡óÎ!°'?ø¬Ö
·ý?n³€æN?鬹ì- À?±ŸäÄÍ¡?¿Újù¿N?¬ØHGÛHè?²À3™:¹? bŠåeã?îF¯vqØ?±‹ââÄ'?™zœáè«á?°8ŸÜ3?¯qI?ŸÆRÑc>3FGL J1123.9-3653@qÁY_í¦a@6Â<à[À9
´br»ßÀ;Œ[™ƒÊ$?ÿ>åCJü@X°få'A?úšÚ\ˆ–¿Ñ ˜Å'οÜëYοáZŒÿ_úš¿íZå˜ÞPSRPSR?cð5øQ÷?qÝ9Ñ
¯õ?ï»*à>Úþ?‡‰ˆÒ¿ ?xrtä'ØQ?¨ƒ}Âk?n7iËzˆ?€;O1¨®?ï@"[.7?Ÿàán'˜?"(™ç`Éë?œ˜;YôË?¡fØÈÑ÷F?"¹užÒî?ìÇò¹Ë–û? Ñí‹Å?±ýÍ:L{?šE>ŒŽ€H?"E;)Ú?†Ð'û֌Œ?î4¨Ž^˜³?žϸsŠJ?£ٙßÐ?–dš%ƒ"53FGL J1124.1+2337@kDÛ@-¹@Q€%ߙXÀ9ºJ«õ¼°À;ÛjÕ`ð¿ö9ühEä'@W©¯¼EÁ@¬=?üoR¿å(þ§Ê¿è‰.+PU¿ßžo¸…Ô&¿ê®ûC€AGNfsrq?ï¶ky^Yà?'eúkÝ€?ao»l
i'?i2?D_Î?|ešÌ[‹?ŽŒ @ˆµ,?︜bñ_h?'D×Ï¡$?l²	Ï@X)?s5+à²~$?uXɟ° #?y˜_•±²q?îÏ-OÙ3?'Y¦žÅ±?‰¢ºm0§¹?ÃK­œD?™Mýl…¡?Œ›Â'
àr?ï­~ÙùÚ?ƒ«4WÔ«?Eê…Ù]oz?P†X6^@?ƒA¡#ó¥ö?'†ÈN#¦ï3FGL J1124.5-5915@r@@ Ç?ü5:ßÏÞÐÀ7ƒ¸µ¾"NÀ:|{üР—@&,§¨Ðï@¨Ù>Ú[@ƚŽ½¿ßل ä¶¿ã}á·aøæ¿é[J÷š¿ëet®/PSRPSR?I¢'l®'ö?UL˜Úó±u?ï.(Kw5?§ã$e|Î?™måc+¨Q?§Õ%5t?Lq*CНY?k`–T@õ?먏³w?ÂÃIÞÈ|?Áä왁a‡?°öœî?­hOùâ?žÉ†7§y?åj@Å_Ž?¶†'XUí?Ñ~uê<ɧ?´ƒGµÑ?\ïÎ"1?Xg©3èÂr?í6}©aõ?ªªíz³Ç?µØXº¢£Œ?ª^³½	ÌÔ3FGL J1124.9+4932@c4ú D®†@O /µÐÀ:dpA±{8À;탠Uu¿Õ.Bç
ô=@pG´Iž/?üل`wd¿êÛÆwž5¿Ü‹æ¨b'¿Ó›'Uy¿ÃžN¬'ÍAGNbll?ïþ-…0Û>?9fìò½Zè?$˜Aéõ?8!mYŠ[V?)b'l=?'ôwaÞ¤?ïÕR7yß?w†W};mŸ?cúòn{?jÅÁ]Ö?g.æ͓±«?l'Ëñ½ü´?ï<"©O»?'B"¤?€<u3Šö?€H45ƒß?wèÓE)Ÿ?h¼Š'Tb?ïëæs‰³´?`.°ø5Í?]ü<5´?ûÞ®¥?c¨.[\$?_ÖpÁнA3FGL J1125.0-2101@qT%à.©a@BÀy`>.9À9øŠ(Ž"À;"ýs]Å®¿'½É;²Y@
÷áíEh??üŒ»à@r¿ï`ó˜ÇZ?é<Õõ"@¿â8Îò'5Š¿ÆÿxñƒeAGNbcu?ïɔ×÷Y¾?x
Ÿ^Ñ.?\
Ø
ÿ1?Y³qó?t3O¡z?uÊ_û?ï§ÿøšZ?…æ4Æ-_–?uSÛonDõ?{µ°ø?v¬™"Dì?z"Ђ	Q³?îö¹j}³ô?‰|²4wPý?‡´7Ԛ8?yÅ4•Y«/?•N¶ÅürB?ƒBûï¨Ó€?ïUQGÿ—?'eÊä‰Îf?'Á‡ˆ†ÐŸ?ˆI. ‹z?‡ê&w·I±?ŠÎg&ÞN3FGL J1125.3-5824@r=y?ò^W@Î0àµÃÀ8ôËá©ÔÀ:§TÚLè?ñ¬·xÒ¤¨@
ÆG²œ@‡_ZX'?í´…hñ¿æ[›l-¿ßìÅÇ¿íV" ÞÇÌPSRPSR?¡QrÓž…?¤Y¼,ãa?ؗúe|I?ÎÝ2üC#ž?âžëϕGó?ÏU
¤E˜ÿ?ÀѺ5J×?Ä7¥&Ôh
?Ö©¼ìqî?ËGíáʄ?àȼ}¼tS?͝ç'%ª?Æ5Óâùœ?©h³Dهà?Ó,zÚpE_?²g^Ñÿ^Õ?àÜMš	—)?¶2'.q¨å?¹—œB&p:?ª§Hqã?Ñ®[!;'?Àœha?ä?µJ*"e?ÂIšhÔdÖ3FGL J1125.5-3558@qÀ» 1ί@7»'ÿùJÀ9LPtTfÀ;ZHþv"?Óɯ
@§²@h"qM?þ"tÿ±Pš¿Â¦¹r|õ¿Ú·µìêD¿ÚÈoT†¿ÙZÝsZAGNbll?ïû/•1–?:%áOS¦J?*œ'Žà?&-®'²å?9<Ž)šZ?4K%rcn?ïÅñU.…}?~³'
~?g'>>
Æ?iE\­¡?q>¶I¸:á?v¢­9—º?ïQÞ?
"ñ?…¢EìÅâ?'dý¡þ?{slÀë?‰#ñ,¡!²?|¸œ¬?ï1MúLƒ°?‡D-«Jã?N­!kîêK?Pçk›v?˜à׫~?†ær[̨!3FGL J1125.6-6012@rG[€#¦Î?ìû8ÀcïÀ9*]ÔÏÀ:²Qaòc_?î%%‹ç@ö%ÍD@ýÔ¿_{ç¿Ãîü'Ob¿æ̑'§†9¿èT–cjnÅ¿ä25w08,PSRpsr?ÓjWÌÆq?ǸԂÙL?ÂËYõ ¬H?À¢¢O>Õ?á—þÑq¶?Ì;8I!€`?¬mèÀUã?¸O\CÌ2?¦â7ÓîH?§qÌøC³?ì×#P'k¼?¼CkûKCP?Û»<¿Í?¹\ýŸûbn?¾ñq—
…€?§l‹t* ?܈g†­žÕ?¸åW'?v‹?Övf¬$'?¼ú‹¾™
æ?´TºÄÒÂ?­Ø	¿o¸ª?â:Iҕ ?¼Çª—£3FGL J1125.8-0745@pÒäÿÉy[@H·&_æ¥À:oæÃ%À;ÎCG}m?'É£a>jf@ˆÚY¨=?ÿB*Z~&¿ç­¨,·÷†?ÒwF™¨™M¿äÉns{"¿ÙªaµEAGNbll?ïÛ¼Ží±Ù?p€)'?[3
Òb'ý?]r	8÷V?f©ë©y?i™§.<í?ó¦ž?ˆööÅC¦ý?y´¶Š?'Ÿ
Å?t¼Qv&ü?w¥u"îzj?ï#²ºûù?‡Çee,?†d€(že?y$,k½~?†Ȍ1y?˜‡§½í?ï?£³Aw^?Ž1?†0*¢?ˆBó]'0Ó?…É_Š9¾?‡ÔÒ÷C?'c¬WC:—3FGL J1125.9+2007@l`xÜ@QO?Ï"èÀ:k™èsòÀ;÷úŠu9h?Þ[g/ö#@'ð=?Q@}?pÙ1¿yt]þkˆî¿ç	Ž8f¿Ûš+5Ÿy¿ïÿÎÍ&ÌAGNfsrq?ï° ôÐÒ?ö~ߙ†?{=¯£wU?‡'ÛµüŸ ?ii¿«è>¬?uLoþSÞ.?íÞõL"
?±í,ùb÷?¥bŽíK}Š?«@UªF?™\0؃L?wå}tÞé?ìS
œ(0ú?¥ÊÛ¢ÅC?±r|&¦È? Få}õÍÌ?§ê-ð0¼Æ?š)1iÁh?ì-°xEÈ?­Íe¶{?²®\õq™Þ?©DŸSê7#?§È>ÀK?ë½gÑç3FGL J1126.7-3834@qÔ_'`@5aTÿ5Õ¥À9üËE%¤À;µïXz?Ü{Fþþ3ˆ@ým"V_@)_ÊÀÙ¿¨Wx6ó\.¿ãü狃Æ
¿é¢<a@ró¿ÎìAÁ/N'AGNbcu?î1ýÍA÷?¶žb,ïĚ?§ªyË]?³Ö2&1[T?"ÖÖ½'
ë?ž*ÕBuJû?ï‹à/
«â?'ññ`Æ?yA4ð…É?~D{FÕ[?€Ó¢Üĝ?ˆ®¿Üúó?íñ1®-'C?Ÿ·D¨ßp?¡Bæ®ï=?—Ùø×Y '?ŸSüÜq=¶?‹Y0@ÿüë?î"…4½?£É'2Áµ%?‰¤ë,1›:?Gk›>Â?©tœá§Çp?¢)%F¤Ð·3FGL J1127.0-1857@qK…ߨq¤@Cʉ€Fâ=À7R_IÀ:æ3hXÔ?øbýPMJa@ð"gXSÔ@/8Ç¢¿àD¹¦h¿ä@W¡&«»¿åC¬':׿æ¥N…ÁlêAGNfsrq?ïív/'Ø?]jh³÷j?Mì礋?QzW}Ÿr?VŸZ†|ƒ?S/'}·¬ì?ïÕJ|¿•?vãɊZÛ?bۚw^ ¹?j#\QÌc?gÚFâIS?mVs~+W?ï_p2ó0?'°BÇð¾F?Ž_9ù´?ŠL`Y,R?çĹJ"ú?†&»Ã}‹?ïæ'}š½;?u'weª#"?!Vû¾ÕåÆ?FýK…|œP?héUeÃ?u@âSÇç	3FGL J1127.8+3618@f‹-ÿ'+¿@Qƒw`MÉÀ97¢ô§À;¢1¿•¬¥?å,>>v±@"¡Ì@Ë;\_¿Ùúö~ªˆˆ¿ç+Q í²¿åœšQÇÀ@¿ã3÷ã?Ä«AGNfsrq?ï÷쟌?[FiSŸH&?;#¿W¿2?:
Õ³J@?B½þ"$¡?ZO'Ôû?ïÕaª}?ó?x?VÙÓ¼?aà~¤E*'?i'"5Qs€?h½ÖÞzã%?o¿R쥏/?ï!Mq!ox?‰jf€`Ð?†ŽÓ=·?!´¦
°?ŽèSÄñð?€x–Ú÷3?ïÑ>7Íü?wè¸ü?F?B:Ñ:ŸH?F&úfªŒ?u‰ñÀ¤¡?w">¦£à±3FGL J1128.0+5921@a§É`0Â@@K[€"ØÀ:hJÆͯKÀ;úÚa
¿é†ƒÛÓa"@
Õ´¿%D@¿¼w¯d¿æÜkûõ.¿æóý¤lA®¿ìzmôWß¿ïÿK'$°AGNfsrq?ïÞòó¿Š?xiªì³'?e>Ö-"pW?pÇtNé?YPm¾<
&?gƒGö"õ?î‡×+8t?°@ŸÇ[ýI?ŸvØç7õ?¬:Îз?
Ccrì?"!w¶bÁ?ìÑùðhC?¢F{>ó‰?¨ùMŸ1Âp?–}DMU»h?©ç^ç¹S?˜+Xæa/J?ìÏðÆчñ?²{U <?­$e€@Ly?°Ó˾7£?¥ÜŽ§4m?žÇÄÔÒ3FGL J1129.0+3705@f>A [À@Q~³Œ¼À:Rîº]À;ÁXù–Ys?Ö!¥Z@8É˳@¨Yÿа1¿æ^µÀ@ÍP¿ãp«ëº¿Ü(•kÈ·%¿åÌÔkÉôùAGNbll?ïûҖB¢–?:a½B?-Žƒ5?]ÇVŒòI?<êJ)|	?8Qð
ÉÙ-?ïȈâŒ?|^Ӊ§<.?f7ܟÀ?kÜ©—‹ƒ?p¸srË°?uçáéX[?ï©9ý7êÌ?v}Üvùó?kÑó‡Û—2?d-Etõ"?}z Ά?qÉRÞ~†?ï¶ä2´¥?xƒÀ"gV?Qtgd$ö?RF¤:é?€#DÒ¦R?vÉãü3#]3FGL J1129.4-4215@qñÂà°«@2nÀ§û\À:ŠÉòý¹À;¿IÍ©kŸ?ޞÏà
Øl@U¸™9@ݵ_Ƚt¿ê<âcâÓt¿ÖAéV<Äú¿æ/–àÏ­¿ïÿìã~Ñ(AGNbcu?ësú–S…?Âê1àÆÄ?¾Ô¸/i9?¿8'µ–	?™Ejìwêt?°Á(¡Rþ?ìR°¤:‹ü?´úÕ‰(­?³,*ÿÓä›?¬gÙ4cE?¤|Ÿ¼¯vû?§ÕŸÕ5[/?é'ú:"´?°qÏ}.c?ÂFùMÂ?¬ð1c±?­Äwö€¯e?žŸ¬f?é,"'ëÞv?²ÕéR	‡ï?ÃÑdš"?±°Ñag}Ã?­ùµ>Ú?›ÊqSVx3FGL J1129.9-1446@q3nÀrKw@EÕñŸêìsÀ8¤˜ÒÊ<ÐÀ;•¯,¨Õw?èãà:5@õ`ªåœR@Kà˜†Ÿ¿è.&Ãۃì¿èTB齿ìUÂõ]¨¿ïÿÆւqúAGNfsrq?ïü¶Âní?6§Š¿üÒm?28‡ gªN?1Ý·n]C?#s…˜A÷)?"¦æòþVé?ïÀÀ잸?_«"VÜ?p9w2Â×?vzÖJ¾Ê·?nËòrâ\S?sOñ/?ïx@Ôá?Ž´÷IÄ`?:û½Àu"?"Ï6Ë? ?‡*tIÜA?šaôž|ý?ï¦íy¬ºÂ?…§Üõ\©?p"?áU${?xrûÄzØ$?|gHMz†?+UM9µ3FGL J1131.1+5810@a¹/ßÁœ@Köõƒ¥À9üÅ0÷ÑÀ<¯k'ö¿Ù xA@@+­,ôU@EP¿`'³¿æÏÇ~f¿èkçÀÕ.¿ÎÅýtNJU¿çÎ^G^
AGNbll?ïÇHq?¤Î€Ð»mß?c{õ'ÒÕ½?'Ê¿sdO?r÷á^
4?–ü Ê'à?ït
žÍé1?–ìêén?'ÿCÐ4—??'­ì';?ú¨ø¢9?'¤Râ®à?}ét?"Ç/SˆŒ?"¹•L+O?~Ç:šc`+?"2‰ü;ê?"}h¬Ó™?ïg(¤Hc™?B{B÷ôÆ?]œT±ý­?_"Í¢÷©?'Jᱨlñ?‹ÁºKÙñ–3FGL J1131.4+3819@eÄ_Js@Qv‹`òËÀ9Õô†O9úÀ;?)
»E?âð—	qmÖ@'þ'…@"@ "€¿è¦qYg-¿ê¬Ü-Ë¿á¢Ú- ¿ïÿÞ\
¿SAGNfsrq?ïÐÕ°6ÿ?{6bë	AL?U–³½|á ?]8€o±?r/Ǹ…GØ?xïî՚ü?îV»áK>{?§Sôpm÷,? ZÈ=H? C2ºæº±?"ûÎF9?˜ZRâ?î"7¼v?—ò{v\3?šË±U£?s?‰áJtn=,? v¶Il¸÷?'w¤Çxw?ê¨
OÕ>?°˜@&E?·ƒ½]ÐO"?ªj'OSÛ?¸O±?¤íŸ38C‡3FGL J1131.9-0503@pÒ: WŽ\@JC* dúVÀ9‡;±†ö)À;ž ùt̿햼CxÕ@'
L46@D)ÀmÃÓ¿æ
E")Š_¿ë/gzý;¿ë
r.¤?¶.w•@wAGNbcu?ïìx
¬0ì?aȗ¯âS?Q,Û÷Ô!v?Rò[`öòÀ?Uã¯Ê	<?X"°ÞÉ14?ïÄG:Ò¦_?"7þ$¼?oh©+ùß?~m¶Dl>ë?lP+-¦{?s
4Þ?§"
?'ÁSi*J?‹"ð´GNn?€ƒ,Ÿ@Ÿ?ú³{÷?	èz¶r?ïÃÊf}{û?cߐ;? w5ÒÛ?3h¹6û)*?}—·™ª?~õ'ð/ñ±3FGL J1132.7+0034@pƒõ_þmY@L´Ò_³Ä¾À8x
è³³À;9]¯Þ}?ãÛÏbíû@Æô÷ŽAw@™ _Æå¿Ýߨ¢J˜¿ã	¨ß'¿áÛ£'¬§¿ÝF‹(	AGNbll?ïòÔ2—¬?QqjX—,??›ûPÿ"?6ñ0¥mäì?RpºÑÓ³|?MϳiÍÏ?ïƒJÂ#QO?úœ~CÇ$?€m}7—˜?"qOÊbÜf?}¤íè)'?€
©ÝO{ï?îá|ì 
§?"€í¥ˆ?ƒéQ¡²Åˆ?|–É_'®²?™Û¹«$èy?¹vò}×a?ìe 1ÿÇR?©L$Þ\>?"µ'¢œà?'x¾"U§ì?·©™ÇZ¿7?§þP±AÈð3FGL J1132.8+1015@opÛ ¸l@P=@GDÀ:gÍÀ;È©lut ¿÷EJ!ŒAÂ@
¶ža@ÃÉàhÚ¿èh ¼IX¿é…®w™‹ú¿éˆíñ¤ac¿ÃàJK0]žAGNfsrq?ïþtÊ÷©?+HìmÁ+Á?Í<ÂÌo,?#Ò
žr?™€>€?#—b¥UÕ?ï܁­nV@?u|‰¦öØ?YŒìφX?b…§â¶X?f·Ü)ær?nÃc&Ò#[?Üš-?{Ӛ¦ïü??sr­­c?p^}Ûª?ƒßñž?uE¿u" ?ïðý×N^£?a!ð$>ç}6챁>ór],‰ã?]ÕVõiT?aõ?tµ3FGL J1135.2-6054@r\åà.©a?ã@?éØÀ7ÅÒtwÀ:°½L&I@‰uҕ
Ä@²,ðÎߢ@ÆÄuw¿ÝxdVRg¿ããõå8Ã/¿åêybru¿ï
$p:PSRPSR?@êÆsýš?@6M:-ÝÃ?íéò"ÓÏ?±ã¦>Ưš?°Ž™\VT?±Õ–Ѧƒ?&qÃ÷颓?9Y!ÔG?ë"H›'…6?¶q3ž®‰?Á­A ÷ð¿?¶qwXëþ?¢¦Èw;ªh?"Ø"6üû?é!Ÿ¶'å?²ó¡~I½?ÆÏÏ	•
Ó?±(Ï_Ð?u0êHù¬Œ?kËO]Å?í#7Îøîì?¡>E
ó¯?µ"2ã¨íÝ? J5:Žõ3FGL J1136.1-7411@rœn «†À(+Ö@éÕÀ97oJ:¶µÀ;vReþaš?é"ú|C®'@
{JÍǟ@Þø 7­ì¿äÊ<'zÿäi˜¦ï1j¿çNµýƝ¿ïÿ¦CK.RAGNbcu?вtVõYÍ?Æ=WN½Ë?ÙùKr¸zž?ÊE¾÷ZûD?ÕT@6R+•?ÈÀÆÐ0Kš?·ëÁjŸp?·X-½Óå?æ;xY©?Ä»º~ÉW?ˬÔ×ɤ?À˜šZ•<?äH¬éº?³=·½rƒ?Ë+¼nþ?¯_ÉaŒ;ã?Ä» ÞKž?¥†e€Ö>y?ÈJ"ªÂ;Ø?¯¦¨0v½?ãUþ&Úo?»ávóçã¹?Ê]s½Zl?³ºövö3FGL J1136.1+7523@`#W`9%»@Diœ@=òÀ:Žã]2À<*rÉK8¿Ô}聴 @ßF&ñ}@h³ UöW¿ì5=Œ«¿Ü£CÑ9Þ¿µ¥úw™®¿ïÿeiûØPSRPSR?ï­¸C;¶™?'ÄGŒ@3?=g'Ê`>?ã=V%ö?Z¤@J?Ìh?jáغÛ:ô?îÞ©n
L? þæ»7€_?""WA‰†Ò?•˜ª~˜.?—zûU/¼?•kݽÃË?ìNôšr0?¤-§gá‹ã?° Œ?ÏžÍd+?ªâƒÇL¬?šgöB–*?ï<~*Ѳ?'×°/TA ?q"c$ʏ?uߟ¾¯S?"aôE§?üdѯ.3FGL J1136.4+3405@g‹y¢ƒ@R`×óÀ9ß]ÂSÀ;åðL-Õü¿òƒÐ&žzT@½e{C@ ¢àRG¿çƒvãÈM¿ìWDû»*l¿ßýx=uα¿çQB,Ë:&AGNfsrq?ïûÔ!º@Ò?@ؤå™:?œKiµø?–Ç=d§™?;\û`?>‹ÑmÓ/?ïÆ^'éƒ?€Üò‡<?eïK·`‡ô?pÀì¶>(y?qÙF™Zúj?v«æºWÕu?ïGðÏ8¨?ˆÛ#ú"ë?rW©±Í}b?oš^ˆ?'lÙ¥‹•?‡—x·Ã|?ïÇDä[~ä?vRè|X«?3;‹j	Ÿ?8—ZC2ó?{)Õ˜œÕ?uÛåɐù3FGL J1136.6+7009@`|ŸŒ¨@Fӂ PˆÀ8Û°hjÀ;^R_Hdô¿íxGøI)@²ĆW?ý-;·¿ÓFãh3‰ß¿ßºˆÔ©¿Ü";
dS¿Í¥+OO7AGNbll?ïs
'?ÅûCLÑ?vnÌK?vº`ªO?ˆ
S¯Ë?›ktªpêË?﶑€Þ̵?'ÕmUï#)?rÏDµ]}Æ?xñоù6?qçúÛ<'œ?tÓ3£L?ígæÀL2Ü?€£Ï1?qÙg7«?ß{ö¹
B?ªÈ§G¡Pl?•U¨t–mà?îÎBԚR[?šËéʖÐ?IQËé>½?_Tÿ°-d?¢¶‹Š5^?šjʜ^Òp3FGL J1136.6+6736@`®.oKè@GûrÀü¨À9À®9À;"Í.œ?Òוù&@gғ`DŽ?ûe?õ¹U¿ço@Aä{ë¿Öà0^l¿Ó—öÞx5¿ØF€i"AGNbll?ïôC>
r@?Wx$©èF?D†×{ÐS?SŽ‰¿cq?Jlþò»4Æ?D§*ylµ?ïš`.+']?ŒÔÈ<?|$d*æþ™?ˆX*]…?v«"¿PRÄ?wt8úW‡Ö?ï^ÐF*'?'ò2>.«n?;<W©œ?sóX ü?ˆ®PM ›'?zò㋾«?ïÿ×I'ì?Œ®ïÍDtÕ?dõã$¦Íú?gAÈ ìa"?šH²8Ț?‹pí'JÑí3FGL J1136.6-6826@r'?…Q
À=™àvpÀ9"Í]"ÍÀ;$É3»o¿ÑW R°Ñï@0˜ZT_S@¯nàˆkt¿çRšNÛ±¿ë>5oÎo¿â™þƒÔ
"¿ç4!ßñBAGNbcu?ê [yš&?Àé¿GÌ?q sè1ð?q7éf2ø?ÄñŽ|¤é?ÀÏç¥U9?çùËƬ¸1?ÊðC·=â?¢k.…üw?¤âzmqfÝ?Ë~CÎ_?ƾÞÏâìµ?éTké'V?¯¹{¯
û<?¨÷Õê•?'¨ç4¤)l?Äp‰™'?¬"…'º?èØ/ª
_?¯;ªíWx+?€±B¿Åtº?v«Öåý?˔-+Ã7?¯H2¶Ÿ"ó3FGL J1136.9+2551@j¡Ì Õbž@RS&@©À:e¾BÆN.À;¿þraFl?âeë^¤j@}þraF?úÝ[ d¹é¿ëœn<7''?Â_âfšœW¿ëD"†âÝ°?á|«¨‡@AGNbll?ï¿nü(öd?"ÝÐÄ?zý)©Ì?"7¹s	?U-aâË^?X˜ì£†ì?ïÆñLŸ¾Z?'ÿœñ¼?g[р"Áü?xo~,ÄUl?pÙpïÖr&?uZ´‰¤ž?ø+.™?•Å¢ÛAٛ?™Ü|ÏK?'®açÆç?'ŽÄñÊâ?ÓØ2Sêà?ï¾fìx¾V?ˆ[å¢þ?jX/ï õ?×ÍtÇÄ?s r@)D:?€ÐVê"3FGL J1138.2+4905@bÙ`Ëò²@OðÓ?­"ùÀ:U:ûÀ<Êý¿³àÀYI&‹Ï@1#õ'´Ð@Í̀{æU¿êÿè¿âxnùÝÒ¿ëèé¸ëÄ_¿ïþÒ
ØkAGNbcu?ï¹´Ÿ¡ô?"a/W96˜?6cÚ³ØB?"Wœt—A?0E߬uMÑ?9"Ãèb?ïÓÑ_{ð?{·´<Rzº?bãÄ3#¬‡?må~€ñ?iK0m`cv?r-'1ºw[?í¾TÜ4Xt?›W5w‹1Ø?¦÷T¸ôEê?–^
	:?šF»Œe¿?Š±+;™Uh?ïòFȔ&?mPය?$ÛM¾Øó?M®¯žèVø?XØheÖ?kîZãM3FGL J1140.4+1529@nM߆ã´@QtUàeuÀ:¤ü4µêÀ;£ÀÌäJÀ
/0ÁƒÃ@	&z?É?ô $ sRˆ¿ïÿè¤Þ`?ï䉗mðH?ÓùÊÁÚ«]?™õ÷­9ù:AGNbll?ïü·òÃr?>f2PaÇ;?Jµx†[®?"R¥&!Q"?2í¼†MóÔ?:Ë4ɂi?ï×)¶H¸?wþi"ƒ?]µ/´¬'l?g"G{"â?iû±Ý"þe?q?…f÷n?î3ø"¯§Z?£ ""½c÷?¢…jBj¬?¡@œJRî?•Mⵆ?Z?sI%2S¬?ïù\xOŠ?Xìù/#^>¢–ö"¦g^>À§
•M†?J‰y2e?XëA—,3FGL J1141.2+6805@`'na«@GÙw·À:%¾<çÀ;ò… ¾Q	?ç`jŠ¶Û@°:6?ùÇ:aOÑ$¿ï÷«z9#…?ïþ9tüèZ¿Å2×BÇ{¿Ëå¢oÔîAGNbcu?ïù_¾uJ?IbþZï
ß?@¸‰‡W‰Ï?C,ˤV¤þ?3ùHfš?6ËÌ#‹°Â?ï¯ø'©cD?"\è7'?w¯ßl·Ù?~(€«¦OÞ?pS×?;¦^?uþ	9?ïPFŒó?‡´‰èÿ?ƒ4O¹Ù|ù?€´±óî
0?ˆÉﴃF!?},'øƉÙ?ï¢ïònè¿?ˆ¬†È>2`?}ÙØöþ9?ƒ¿ý¢ê¹Ô?p®-эg?w¶ã3Ÿ33FGL J1141.6-1406@qg¡Ո]@Fµ| À9ô¤	_$SÀ;¿WÜ_çÇ¿àǬø@&Fæ™R@gãà¢J¿äþøÖ7|¿ç†?
 Á¿Ö¢uµ'®_¿âêM{³Õ…AGNbcu?ïeùsPq?šl¶¦ã¡?OíxC^?VÐÀÎ0Â?'AeÛûÕd?™
6Nw÷?ïšd7Þ?‹	³áæ¬?{{m€º?'-²´ÞÓÊ?wÜÒwcÁ?zâuz/­´?îºð?¾e*?'«lâôá
?…É7jß°1?ué7¨p£ì?½\R€?-êVšI?ï*jÆìYF?‹M/M¶ê?TC•(Þv?V"²+Ķc?™rBé"I"?Šq•Õ&Â:3FGL J1142.0+1546@n'¨`ܹª@Q"ßÔŽÀ9ßÞèXÀ;´¥hõX¿ÿx9ܾ@2Qç3Ö@^È •¡½¿ß}3£VÂì¿ä€Óð,£L¿äãތ<å¿Ú1מ7
2AGNbll?ïØ[ܦS?s![&ž?Wm5ۅh?UÏáïá?l3	ŸkêÙ?p¥Ràâþq?ïÕøP?y$£ÎÖ?_ÿÈÇ:?fÏkÒªr¾?jy#ç˒S?sßÕd ÷?îŒ ‹:ù1?•û$~?'ZK"Å%?…ˆ—0˜Ÿs?y"M¬?Ž²;lµ•?ïÔ³Šª?v§ÚÁ>@?qÅkÚ?.c}z ?udµW•BY?v"­A`¦C3FGL J1142.9+0120@p¹7ß (@M·ç 5)­À9Ì·áƒ=7À;Õ§uû.à?ö!sЇA}@
«¼±Ì–?÷Y©™èt¿Ù™‹Ð5ë}¿ÎðCgó7¿ÜN×+܎¿êÎd~§[PSRPSR?ê]úOÎè¨?Àû‹`ïîu?ÓWAזŒ?À
Óü»€‰?—¥û÷f6¹?ž{!Y?ìZ™$?¿'òÐ
—‡?´CŸWs­?º¹Meý?¡Ïð›¾×G?¥GLêI=?à[.Y<ù›?¸âG€
Z?×RÑ&è•?·'ÃêwJÙ?¿ÛHšuÞý?ª=
Z¢?ê(È7|[?¶™ºòÊò?Â}¨EIon?´ŒkÚ .?¤ÆÒgb|†? *V¯ÙuT3FGL J1143.0+6123@a® ý;*@Jïä ()À9`¸K5ˆxÀ;ºÜ8zšÑ?ìX€ŒNϾ@}ö۔í@+¯ >ŽÜ¿àFc'²°Ó¿Þ¨ÑM˜˜¿Þ	©æ²•Ù¿ç?+õsAGNbll?ë6{Ïæ¥Â?¸¹%2?³˜ïsÀ‡~?°R Ùð?²³2
Jl?¬W'Û?èV¿¥¯?Äíºè®?È·ô¶?ÂÝ]<™¿€?§¸=Y<$?¤Ú…¼·Od?ì…/¦*?¤Üâ´z›P?ªþ6®8?šp…¦ÇÄ<?¬°€×Îï,?—–"ØýV°?æ/•yœ?¶¥›eX?˧>GEÞÂ?´:'1³?·8¾Å¦-œ?©á¯U8õ3FGL J1145.1+1935@myA HàD@RBî?äžÀ:Š"#8mÀ;õÙ&wc?®ÒDHî×@
ĎH­˜Õ?ÿ¡7€ô7¿í+ÈÐé¼ó?Äé3ÍY\	¿è±Ëi W¤¿ƒõ­…x"AGNrdg?ïÃp›*œ?ˆÖÒnpù?x
rpþñÔ?ˆ6äôäm?X×U®ýb?[än'>?2Í-æ´?‡mӌŠ?o`§Ø>ó,?›á€º\a?rE|í-*?uá"R'ôÜ?î§-¼
?"#Šls‡Ð?'ýÀ•gzc?ˆ¼Ã®"îã?˜ Y³â_?‰ºJY'×?ï ®Ö֒?‡!c–=ú?wã0½¸?'5‹Í÷"?xâÅcÖþH?|;{gqSÙ3FGL J1145.8+4425@c}ËßÒc@Q[ÖÀÀ:ß­FÈBÀ<B‹•ÊØ¿§j9DZ`ß@"óM¿üZ?ýšRaKÊY?愈bBH¿Õc8ÉöÑ¿ä:kc{O'¿Ê…û¨¾‹ÓAGNfsrq?ïÝ觰¿Z?ryœ¯ì?gÂÌåÒ?p—Ê•á?Tª‰žçj?Uæ[×–?ï·TÝk³?"	žñY?o²}Èöu¢?v¹Ê5öÈ\?t|¿¬ÎëM?zY3´)7?î'
ÔbT¸?'^PÝë?–ìqOX¨Ó?‹o2'¢µð?–ò4$\À(?'¹+ ?îç˜ȪV?›©¶s2?‡§Jԕ?ŠîcÆAü(?—'+¾ÅJà?—=²Sù¦3FGL J1146.8+3958@dŸÙÀe¶=@QÝ­À,«ZÀ7ê$gMÀ;[(fP–ñ?î'l ö«Õ@óN¸IÝð@çÀC&›¿âdTÆßV¿å14œPz¿å^›ÎÔ¿ç蔘AÅAGNfsrq?ïö`ƒ.äÃ?KÁ¹õý*?FÔ'ß7?F¹üÝ;îr??SÃeyÁ?8âyºip4?ïÚÝVƒaº?uo±˜ä°?^t^Oû±?f:U†Â?eèzT mw?l†Jÿšéÿ?ï4/ºJ#?ŒÌàvôþ"?"@%N(³l?'z<œÄ¹²?Ž³ìNˆY?ƒåõfU[A?ï÷xöpv?\gn?øãŸ?	ºy§Ô<'?e‹Ž°ˆ?Q:Eàq?\-¥N–éh3FGL J1147.0-3811@rß 'á@6ø;‡}À8¦ìAÝ"À;l©èœ6,?ê4G;9"G@no+¢@îàrñå¿á¨g€þÔB¿ä¦÷»oÉ¿â®
Á"Žd¿æBDý¤Ê¿AGNfsrq?ïôj3#Õr?Q²ê¬Æ'?@®jªKáõ?A³Dmáhù?M¨ÈÆ^V?KÆ´Hì
Æ?ï¤Ú-ME¿?†]0!l?qXÿ+©™?qrÑüҜþ?|9ê-´×?'ÞÑýŒ'S?ïEÂZïÉ?"·
!¢2•?a›ªˆb?v]FD¤"?ŽÞ›n÷Üh?	T@Z/m?îê=cö=?–Î{|œc?t/á`U?rÁü<þ{?"Gˆòj?– Y¤ëˆ3FGL J1147.8-0725@qJJ '§@JÇÀ'áÀ8ÊoÖQ°ÍÀ;g9
É<?Üú(t,;Œ@íËA\k¼@‰V  žñ¿ÛÏ|i¿åå»ëpk¿ä®<ì%¿ä(ï¸_,‹AGNfsrq?ïû?ãcÂ?:ؒ©qÓ!?19ӝîÔ*?,ǺéÜ ¬?4É¥Fó#W?2&ŽØ6ú?ïϏӋµs?Ô$zx¹Q?gA"8a!ñ?x€ ŠMÃ?i/
;ékÍ?oÜÞ–¾?ïC…'Co?"ë@]!ô?€&¬S³Ð?u£«öZê•?Ž÷ï\›pp?~Q¦¼®=?ï¾>Œ?î½?€5^zzë??˜'–,?B×ÎA.
?~ç9ßx?úGÓ*í3FGL J1149.5+2443@khÌ Õbž@Rø. &{•À:SYäwä=À;êúµ=d¿ù"øzût@RK»jNÓ@ã"@>^Š¿éI \ŽBÆ¿ÔmPëªÞe¿ç%+~ðI¿à±60"›©AGNbll?ïïƒ.x3|?c7¡fgõ?O¿þ6•'?T&°qÞ?Q}¼ä?[›ƒåÉi
?ïÌFžªÒ?%m	1?a܊_™9<?k'…× ?q—€Ýú?|Þé%"D?îú$€0÷·?Œª]"i?‹˜z>ý5?~øÀ¿"ú?".£¼ÁŠu?"³1gž£?ïºhp8Qî?yu\¾‹Ø?2Ò1^¾§¬?;ध?€ÏRfõŽ±?y/F8J3FGL J1150.3+2417@k¥Ë èBt@Rþ)¿ìêzÀ8ÛðòFÀ;Q†Xt5\?½×ë4¨Ž@"úõT*z@³&ÿô"¿áظÀrù¿ã•Lo:P¿ÞyLOÂh£¿è•ñÐ"¨ÞAGNbll?ïjö녘?ÁZSzî?r±˜HÏ?tïÿhn¿E?Œ9xú2ˆ?ŒÓ–™9¡?ïE`,@¬Ú?–1ÄÜA?"ô6ÍeÚ?…¶!Î ¯ú?‰³¾"o¬ü?'<Bß1é¹?î{¹œ?˜7ñ¦ø|?˜g¤cFÙ?‡ƒ Z³Ò?ŸðdÚºwD?' ÉҎyí?ìèq3kËf?£ËÜÆîÕ?™^ã*Ãþ?'O&k‡?²d½™ðÝW?¡ãÕý®^3FGL J1150.5+4155@cã{¼¾b@QªÍßòCÀ8P,‰ËÆ=À:î"Z•wÌ?èÚÈ¿™U@Ü"¡À…?ü$PôF¹¿Ñ¦àvo?u¿Û©S1¿Ù
ª©ój,¿Ê=.‰«:AGNbll?ïÌ¡U?–+>êÀw?~,ù6òŽ?}_–"Ë¥l?"»-'X¹Í?'U˜VM€Æ?ïTcé<‹?˜+_ߘ‰?"þ¯å«"?+²,¢ô?…é•Ë2?ŠaLeÊÓ?ì_SüW—?¥ÍŸ¦SQ? b°¤?q?' .«q¶*?¶û­£˜?¢ú°pQh?è,鐜èl?´KÖÅåêÏ?¢]CšŠg"?¤õ•'Ï?ʵÖéĊ?²Ä§žá¬º3FGL J1151.4-1346@q—¢ŸœèÙ@GIZ _†xÀ:(8_ÂÞ7À;¿?']<¿Õ-Âvî°@éi{Ð?ÿ«@àoí¿ÜZ§žó~¿çÁ Hõ½1¿‰s¯,Ü`¿Ýpà~‡½AGNbll?ïõíf~æ?Pýg¥OÂ? kÎóê¸?§'ûÊ\Ü?R%	¹#·?N÷7ùŒ%S?ïÅÆLivº?z¢÷v m¹?m†Ê}·0?pÅ>›õ»?l²éѶd?pØ$˜[»?ï^7âà"?~JÚüÑñö?{"h?ohzPŸZ?Šç)|¹§?vËâj÷á?ïœ`bš­ï?€}Žª|KÓ?#	ó#Uz?/ž\q[¤n?ˆ›¿ŒÇ.R?€n«S¢•"3FGL J1151.4+5858@a(¿;ê'@L>­¿ÁKÀ9iëBÙÏÀ;¥ÒÐçÝ.»™›@PÍåüs®?þ­&žû-]¿æÑØú†€¿ÙíuÝ/y¿àÖ¾ù$™'¿ÊŽ!%–ŠAGNbll?ïô5´»S?Rú•ðœÿY?A›å·|r?;þÚÈÇQÔ?MG\&µ?N:»ßÇß?ïÎßÛGžà?wá=¼*—?fã)÷X´?l°
R60d?j<úÁ	'?mÊQPâûÂ?ïFé?ˆ+©ººúA?"«œ2þ­?€h*/ޖ°?‰š"Mm;?{:ö%ã?ïÆ¥Aç4?tÖ"òöñ?'ŒE$lÆ?1»ãØAÊ?{ðýSl[?tAaBæ3FGL J1152.3-0841@qq_¿ƒ8.@I¶hÌÀ9(ÇôøÀ;"°Švæç¿ÝÆ Ò@""†g¹@Ž=Àâc¿æO&ŠÈ	]¿ær^E"_¿æç$˜`¿ßf¨ÎôL÷AGNfsrq?ïòÞN?hÆĂ7Áj?A²f¹ž<?C*[Ã'm?Qj®Ò.}?fðYÿÐÁ×?ïÀ`Úx»?' "'Åg?p.Q›']?{ü'Æ=xr?oB'«9.þ?s¨'BtÇ?ïF5r³cæ?‰DNó{d?xr|Õiä?pcz¡ïý?'²t9
^?…ëôt/ó?ï{nOþ®?"µ1ý'Am?I4Þï+Û?L'ÂÎCì'?'uZ?"dÊ3D'
3FGL J1153.4+4932@b0öÿ:Þ"@P=ÿ%¿­À8Aó‡K¹<À;–w§×Iþ?éCVqÚ@†@I~úï@A{P¿ãÅxãŸ)Ú¿å"ZíƒÈï¿ãIŸá‡D¿ìÁA_yAGNFSRQ?ïív­½;?Z‹¹ÌýeY?S¼Ž˜šý?RA"'£ë?QV_ëƒl?N«Â Mìr?ïÚIà¯B-?v¬ ¹ŒWQ?_³¢¸%q'?g{_ã]ò™?eÜMô«ù?nÈ(xBg5?î‹X.½b?•2Ië$ƒŸ?—]¦˜ ?ŒgGsŒÃO?—AWS;"?ŒÍ±¶¬ )?ïÿ7˜«Ló?(Jµ·ˆZ|>Æ`±¤AD>äÌä΄ã?[ïÔlÌ?(E"›;Öø3FGL J1153.4+4033@d`Ï‰@Rڀ¶–À:wŽF@À;ÙUËäo?ÍòÒ_*w@Ú[Ü®l?üF!_K??ïúGþÿ¿Ò'¯·µ…Ö¿ÒÑ;Ïíq;¿ÚÝx-Z£‡AGNfsrq?ïôu»	6ó?WÄåÊõšR?NÇ°WÎ["?TábŔØm?>ÂÇ«»d??•ÄÇèÿ?ïtŠP·hã?'·EÓ>]?êX?…	§_O¦?ÀSènG?‡M\²_f?îú÷Õé}?‰heU±øC?PՋ˜ g?€šO#­)?'øš}="?~lH¶Ð÷?í¼îyúTœ?¥l?š7GÒ?™ À–"4ü?§Ž¼Ð-]?Ÿ¯Á£âÑ3FGL J1153.7-2555@qðe¶™…@A"Œ_õ3À: öC¾›²À;à ɤ#`¿ÊF#.§@
ˆùyO!@9 4¾N?ìÕa¤h]¿è"ÍñÔ²ä¿Á7æÁj˜û¿ê8חAGNbcu?ïb¬ZåÜ"?•sÉd±?see"»½?tíÁó«1ƒ?¢6·÷™Þ?"'¶÷Mþ?ï`n«'Gô?'7W¤é˜Æ?ƒÛ•e€¨?€ƒXÍL½?"¿¹íZÓ?ˆi§ç?¹?ìuÐs?¦ žO€<h?­dX±q?ž¥Zk"í~?«>¥gč§?›ÚÚ·»Á?î?ØYêq6?¢j¶3ÉÈ<?p±.­ˆ›ý?r}FmQh?©ìT‹§Ù
?¡ÐñôFÔ3FGL J1154.0-3243@r²gÇ@<œûÿÀ? À91ÃÇkÀ;iEW"&?ï­qpì¸a@I¼ˆ†÷«@lÅßȧú¿Ü‰I±5'æ¿áˆý&~;g¿Ü@Ö²÷¿æ¾üHÕÆAGNbcu?ëLCæªtn?·±ëñ æ.?´r'ï:"?¯*{ÍÀ͞?±+MÛqØh?°'	ïùÆ?è{øE~äU?Â'd3?ÇIñCz.?¾ìé+F½?«¶›ÃÑö?§ïâäÓNU?êçZúw¯?©‰È>þ®?²QJp±¢?Ÿ f•g
³?¶uò·z b? í&ˆð{È?ä_íš?·PdVñV(?ÆʧŽ?³ÚÑÎÜÙ?É|qµ¢	ä?±è_Ð93FGL J1154.2-0010@qå¿­)™@M¶xßå®EÀ9ÜW?öÀ;r¤Þq9ÿÀ|v4ÐR@¯9"õjÑ?úð ¦=¿åô"½Ö¿ÝÜSH¿Ô÷"}~c'?£ÀÌó&JAGNbll?ïü\¯®œ?@üÿ¨x
ï?|zý9o"?!kð¹«<?8­ûÃ<Æ%?>þ@?}7-?ïÝ1¯ÅÀ.?tt‹‡Ú?[¹U
ó‰¬?cj"jé6?dñ¥´Æ
Ÿ?k›Õ0Ì?ïy¾˜õ2¾?†÷!¿%_Œ?~Ç«ìÑ=?@ Pz8á?',ƒÌJÍÐ?z!ÜÂÇh\?ïùÏ4_§?IàW»ÿ>y"]à×9>'
Ô­©?HÂaYÖsš?Ißó;<"3FGL J1154.3+6023@`é¦Þüz:@K¬ºAn_À9‹æYeÌãÀ;Ã^Zÿ*?â,š-±@{ÅËÑ¥$@AÚ?üð+¿Ö\Ù²ìÆ¿èy˜㳑¿ìšý‹ K~¿å$r3µJ`AGNfsrq?ïø}ãÆo?[æʙV?FPuP7?OßY­' ?0g÷,Ÿ?PQ^¡Çà:?ᆰT"=?~}Nk×Î?q1Ez…&?t×ðFª?nó w¸¡'?qÍhÿ@%n?îoVÌ`˜s?•YâŠv?™WïíÈ-?'—ßæã?˜½7dÿ)z?‹
à÷(ä~?ïmòþÙ?¶Ð.§i?uw›ü\6?wÕ¤ºqŒ?‰ÿu´ÝÛt?‹QÓþí'ø3FGL J1155.4-3417@rEߨq¤@;(Ràw¤|À:Š…=ÂÀ;š®]uüÜ?ÚÃèNÕÈk@gD¡D³¹?õ]ß>>?ï†	‰ÍI¿ä–.ÙÃfƒ?¯zH<ý¿ÂxrÜ°3~AGNbcu?ï½´·ä¼@?†×"t¹?0?5ž>‰Î{?9rN_Ò'?ËÀ%	ÃÙ?†¼*Ö#ú?µ$ƒà?–û$»Óz?t}ûÉñž?ŒW
vVúõ?y¨©£Ìq'?†F÷¥p:?îƒôO6.?—þÒ|nÒ?""ò$5rš?ŒóHéñ?›üƒõ‹?ŽÆHl0 ?î%L	D?¥³"Ik:g?Yi{V³þ5?t¼!º(À?¬ßò"¶:?¥wàó­W_3FGL J1155.9+6136@`Ʀ?šIÃ@K%v¹ÃÀ:Ïÿt¿Å}À;÷û'Ü5ö?áõûÏS@8H‡®4±?úVÿn4¼¿íÕĘ©bB?ïÛ ±•'´?®ÅEÞ M­¿àÐ3xl<AGNbll?ïö-dÁ¹9?WY™'Mßè?K€'
J@?UN‹wj#?8eØÎ!«?9gy
†?î§Vb¿à?©áÛRzÂS?œô\B+æ?¤É14Æ»?ŒA®õ°\?'ŒÑÀÓ?ï2ÀÎíÞð?‡t·oM?‡Ó'`ƒ—j?'±ÃVZ€B?‹|¤ä¬¢?vœƒn0©?îŽk±%è?¥(+8à³?¡2z]F?¢o25Ô×Û?‡´{Ÿ]mp?ŒÃ7û«‰>3FGL J1156.7-2250@qìò?î,™@C'.ÿÇËÜÀ:='¡}"À;¢£Ìhú?à`ðúP@
/FB¯}?þ=~`X/l?ï¶z'A&¿äQƒ¯½¿ÙumKv»¿Â£¼y© AGNbcu?ïåƖùH(?m@‹Õtj™?MÜ÷Ê6Ê?^°k)?bÂ+CÅL?f`3)²?ï¬ÕƒÈ¶?"-í;¼*û?s£Šê,eí?wG47™öÏ?uñ´Sï?,?zgw'?îû«$J²k?††ŽdA)?‰|†qÍ?yJf8K?"]3q%¯?~B8YÀ·È?íß3¦ã1 ?¥Î™šK?w¼Þê|Ò¦?'Vªz>8V?¯)´}K²?¤¡Ó¤f›Ÿ3FGL J1158.8+0941@p­ÿ'+¿@Q&^è¬À9•,D+¨ûÀ;˜È¡ÄáFÀ0°ÿç¬L@«=ø9à@R"`R%<¿Ûiís¡Ÿ¿âì3ˆ©Ão¿à©wÍA¿Ò;'§%ãAGNbll?ïûãß|km?5¬£ÜV»š?0"kuä?Aτ,8Ê?9TßAÀ»?3-³Äß?ïÛð$^¡#?uÌz3ݸã?\í6Ɵ%–?g\íQ»Àê?e™@>Hˆ?l¼ìòùA†?ïzÆdž=?~›º³­óá?xÌ–±Ø?p'zéèÓ6?"èZ
*?v*,x?‰}?ïî:(v?aö]yT>Õ¥öQ0åA>ë
")?aîòø®ñ¯?aò*xâÁµ3FGL J1158.9+0818@p°ñŸŒ¨@PÜäÀ™,À:§ÎçY@À;ð?HkÈ¿¾ç­xɕ`@¶õlÿÜ?ýéeŸA#a¿ê|Aâx…£¿Óûãl˜Ò¿ÅwKu
7¿Ù­/}ñóMAGNbcu?ïü'›<ñ?D"I×Sñ|?06'{òO?8f·cæì?-(Í®?<-Ž{‹s?ﺒZ]¡?—º- "?oTÆh±¯*?tÄÍ÷7ä?sNxWþ?w¿á0IpJ?ï/|A·­?ˆÃŒ?yŠh?ƒ=5sçÐ+?{"|V?qá½Õ",?ƒýáânÿ?ï ÿ(Մ?~°ïåäYd?T⡼E?[º ßw? ?…_cá"•?}$ˆ3jŽ33FGL J1159.2-2141@qòs?Èlì@CÊÍ_™Ã‹À8Û¼¸''íÀ;>£
¶¡è?×Ò8ôŠ£T@Cˆ™A/@â矶ê¿âóâhž¼¿æ¡y™ÁT¿æiùB÷vo¿àôÓ;YÏAGNfsrq?ïõ´¯?Mt0äF?<ßjóÜd?7†k{2ö!?J¾NƒÁ@°?GäÂÌ%k<?ïÏ;VÃG?yìÂBù—?fÞÙcP'<?k×nßíï¡?iåÏٛ'¨?s4T¢fð?ï\âԓk?€T¢¬"U	?w'ž³›K|?gººF«¹?:wñ
W?zíB0]ÙN?ï™,*!iÜ?'9ˆE³øÍ?<]tF£Ÿº?>üé(6w¢?ˆÒ	ÕpkÎ?'{é6[3FGL J1159.3-2226@qö`RP/@Cma .QÀ8…ž8dË\À;ÍèU¿O?ñ_ß0§'¬@&æÓE7@ùSŸQí¿å\¯:ëŽY¿äZDiÁ¿äªP!Å;x¿êŽã4îVAGNbcu?ïÏP3ê¢=?r–= Då?pó»nšQ?päÉN=	?]ªpSÕ?[øøumÒö?ï·|"¿?ÊbeÓõ+?rpµ' 9
?vOòƒö¦â?rŒ3€DL?tíuát; ?í|¢G×€?¢Œ7[Wêv?§F¦ÓE§0?›b)~‡DË? ï4²Üàº?'րhí?îڇèû±€?"Ä"l仵?x¥þcb;è?vþB´>!ƒ?ž…ƒG±A8?"çyÞg×3FGL J1159.5+2914@hî?àH@S—úÀ%À75#Â|ç²À:ؽØ=CW?÷¿·e‡n@E|^Jc&@éý¿]ù¿à7Æíî8¿ã"<b3¿äÂBÀ
¿äcåj}wOAGNfsrq?ïïN<?oÂ?f™ØÒu"?CH…1»ª.?CMÛf¹V9?W¿DèB¥ó?ea9¡Ü?ïր'"¦?{h]8•9?[ãÓ$/·?eùP‹«¬Ù?kŽMt[BD?v©—Ýå?îíÊçF»ž?"ß›Y¨C®?ŠYBIiLÿ?†Y>Zö?•òsåÄ?Yïaïc?ïú™æîX`?R ª1ÛÎ>é·î½ìD?…sµÆg?E1"‹ªs/?Rºá¼3FGL J1200.8+1228@pX: WŽ\@QÊ9`~TÀ:ªŠ'¥aÀ;Ò7yê¿Äf!‹Ú­û@GðÂJgØ@üµ?½Z>¿ãɵî¹Ü…¿Úôê-ðÖ¿èäXòµi¯¿Ò €³2ŒAGNbcu?™t}ì?±<Ÿ<ÆC˜?Ÿ?á[bg¹?«°ØD*Ê_?RVìµ2?¡aYc›=ž?פֿ[Ь~?…Él½]?ré%Bo?y&™"ô8?w-Í."~R?yâr³OêÀ?î,>:?š>€F·
œ?›`Ó¨.–L?œ¦Gì ? lÒHGƒm?ŽshðA:å?ï8év'2F?ŽèHlÒM?|>LKyê¿?€G‰­gÎ?'Ó>(;<·?Šê )â333FGL J1200.9+2010@n)<ßï¿@@S!ãŸâˆ÷À:»˜¢úÀ;Ô O*à~¿øâZ=8DÀ@;ªv`¯m@1Œ` ÿ"¿æ0o<+ˆ¿ê?äߓ#¿àvºól¯è¿ïÿåÊ/õ¢AGNbcu?ï˜$ëçlî?«A0DçI?DOšî"?N®W'F?ˆ±Ó\uÛ/?«0˜ÑçäÕ?ï ÷NaÏ?ŠûÒù{¢õ?söûî:ã?zýÊÀ`?{]	Ëݘ?"Ø%ÍÇÅ?îYÆ^§? },F±.Ï?""ÿŽn?‡fÂéEgû?¤"™ZÇz?¤¬9%Î=?ï3—OìW?ˆC§\ÿ.Ê?V E1(§å?iFP"V€à?‰/…ßÕ|?†JåóYà>3FGL J1203.1+6029@`­ñ¾ôœõ@KÑm`U«-À9qɕà§À;Ô#ú±¦¿ø4€z¹¯@²:)Çy§@ªþ¢Lœ¿é<*Fê9¿ÞíÆw'¿á»qä'¿ç™Ä»¹ÞAGNbll?ïœÑ[pß?‡Êõ[ÇÞ?uÏǟaC?wi¶T?{ǃ°S/?€˜Ç¿ÓW'?爫zÈA?†ÿE÷îp?sçX­f?x×R¶Jâ?wT!~yp?ü<~`?îaðŒaõá?—«~ú[&#?•gRìê@ß?‹@¯Ì{w.?žZ›†×	?±ZZé`´?>©H4?ŠÁ±Z¶^?TwÕۋº‡?g‹YÉ[{?ŠKµš<{'?ˆË­ÃQ…3FGL J1203.2+3847@dààëgÃ@R¥ïß÷KüÀ:k'öjÀ<q/îU¿üÐÚ8M´@fÝ°õ«¾@m!¬ˆŠ¿ãAÿÞЎ¿în-{°?ݯ8gOšr¿ïÿöõ;ŽAGNbll?ìՅ˜¡r˜?ÇD³¾'Po?¢§†m¥>?´†Ö¦kš?°Rw½˜?ÁzééŒ'?ï‡ÈbËU? L™ø-Sì?x•&2á?/úßêþ"?ðÊÔ3¹à?•'ç[?éæõ'ƒe©?°Jnª£|?³höí>®ª?¤©&'«?½_\†¦$?­X"-¿?ï•SõTB?'œìŽZ‹n?0»Õ'¤ö?W'ŒLÝB?Š%`֕Dz?'{kaå3FGL J1203.5-3925@rO@ €@6ƒËßgDÀ:2.¸z/qÀ;—øö ƒ-¿½ÄfÑ	6N@
"Z"
kê?ú7Ó@"TŽ?ì;dÐ9=ä?ïš[ÓæF›¿æÐ3¶Xu?¢¥½‹³ŸLAGNbcu?ï	°:Ÿó?°*ö…"?ƒ‰ñHîU?ˆú²\Έv?•÷44þ?¯td^´?ï±w\rY€?ˆªáEHØ?qy¼Y#l€?z(¢'£ø?uʕm¯Ôa?€'ùX°?íÈiqå?›%UD11t?¢Í™ü?"úÁä·½? «ÕÝüǐ?«'¸Cu?·´øf?ªÚ/Œú?›Ì"ÏQ)G?¨^vɗÜf?'Ÿ:Ê?—+Œ¸»Jþ3FGL J1203.9-6243@r˜n «†¿ÖªƒÉbÏÀ7Û5÷2ÑäÀ:*Eå"T?ü$NÂÜ@Sjøœ^p@.jÑ¿á'YŸX…¿åÇVVVu¿çP§'«"¿î'+'uPSRpsr?p½ž˜?TV?hᮁ!?ÑÏãiN?Ê)â•$*?æö"?š÷±?ÊA.G‡'?GjÆEP,?c¬¸¶®J?Ôj-‰üX'?ÂHA€‹?å'np—?ÂRa™@"|?¯¦Œ'S? hÚú!"˜?ÔütFƉ-?¶ÅEç"=Æ?ã‡]{68?¹gÑZ›6?¢	"¬[ß?•Ò>Upr‰?×Ø^Jrè?¹ªå 	è?âó@ßÎ?»7H(RQu3FGL J1204.0+1144@pŒy¿ß~€@QÀ»À5ÖÀ9°ÙQÀ;›¢ø½ì_¿ÒR¢v?«@%²A±%?þ	'€J¾¿çVöو'¿ÖßŠ§ä5¿×tæY1¿àœ²ßwªAGNbll?ïúfI÷ ?C'(÷>°3?,ätG?&2Ð桂:?>[³å¸Õ?AÛù?ïÎ-M£Þ?y5J€¹k}?dc•‡½z]?j±÷‹¡ÿ?moÔ±¨?qxÍs›?V2E?w‹ùÇ?uáTy.4.?n¿¿i©6?€í@BT?o­ö'³Ý?ï¦Yœ(k?{*=²b ?HL'Õ‡Å?H£Éd5V?"äö;tÜ?zSzÚÆýö3FGL J1204.3-0708@q­µ?|í'@Jño`
+ÓÀ9böo]†À;BöÕ®?×ýµ(/@ý4XÍ °?ýÇz Z(¿å0–Ý@|¿ÓP–ñH­¿Ô(SÜ '¿âV[À+dïAGNbll?ïà™:¾Æ?p™zö´?[2G¬!Ó?Y#R6ÜÖ«?aÍÍï0O·?jʖIg$ä?ïh}‡Á.N?ŽØtfŒÚË?…#£7<¡?"
‰Ñ»C?€¼úý}/»?d½º"i\?î*	ïV?" âo€¦š?'½‡Ÿmîx?†Á"ÌÂØU?ž7=´&Ñ?ü?{lú?ìÄ®Sõ?¤&O[½Öë?'Rp¼ûU?‰"T°'å³?µ–øÄ'Ж?£©ÐÉ[ô"3FGL J1205.4+0412@q5»à~í@P&3`<ÎÀ:.
¦L/ƒÀ;͒ûç2?œ9>ce@ ä}m"@!=ŸÈ²·¿ì/£sžD¿Éë17–«d¿î?`Ɯæ¿ïÿ¹‰¬š0AGNfsrq?îßÌf¶Ÿ:?¨ßZsžPÊ?¡
O ?¨©ºyã[,?P…pòW§½?Y}°•¦£?ìÃV»æ‡Ø?½¢Üêc?³l·êéX
?»?o ,Ü?™âH׉¤»?šÛÇ~Ui?êŸ9Ö
?¬çÛ/?Á1K£Çê?ª¾e¨ëm?¡Óp¿ß¯?'õµöÚ½?ä|€%ƒ'#?Ǽ†Eނr?ÕÄâEL?È}Ò«¾Æü?Ÿó­+?6æ?˜¤ræ$3FGL J1205.8-2636@r'=ÀTïF@A"ÌÀ7"À9+v2ŒDÀ;v¢À‰Èk?ÒnKa49@}ýîØ»C@S.Ÿz¯¿ä[8€$'¨¿çÒlÁ<‡¿ç'"±UÖ¿à<|+AGNfsrq?ïòпU'?U²ÖIɍ?;	Q¨&?:Ыf‰Ë?Sœ,êö^Î?Rïý
Ñy?ﲈ'ã!I?€
.? ù¦?q{ÁT`¸í?r¯µÙÇg?u?õº¢?u?*zzÑ?ïVtš£Ê¡?"S–Ùw¬?v9Ìu^k´?hÅ,òOï?Eó^!Î?›­í·Ç?îÉjAŠM?—j×·Ù?p'¼Z§£?o‹j
8Ç'?¡fɘ,I?—ßjÎÏø3FGL J1207.2-5052@r}©ß—ª¬@&ÉÁ?ÐÐhÀ9É:qÀ;{ö?ŒÝÉ?õÛ£g"Îâ@gwñB"@#à ¼Ž?Üu@å£]¿×K".ùñ&¿åÂHù꽿îaÓZGAPSRpsr?·.±—ðé?³³}ü›,?ìKÃ8\?¶ŒÁ¶éÉK?™á¸§ØÀÔ?œ–|τìÛ?ÖºŠƒ'ç?ʚ—FB«?ٝ_z£>?Ƕ3ZOY?ÏP,ϳµ?ÈÁ‹‰ü?ÊÐHý4ö?³*#=ê¿v?å翐£ã?µºÛQÍ©?»!Ìèæ}d?¢éŠå߃?Õ÷òQI?·	b
;kï?á•'i7"×?»Uãà˕!?»zXìþ5E?¬™FHįÀ3FGL J1207.6-4537@ro@OÂ@0Õ€ÐtøÀ:4\÷QÜÀ;´²$ªÚ?õ}h%-a@Gý™Heõ@æùÿ_ò¿ç5§«uª¿¯ÃO`Þ¿âyaÅÇÚ¿ïÿõ³¶YAGNbcu?ÀŠúV~]?Â!‰677v?é'áûrŒ?Ç{ü¤Âõ?³CÚ2¿næ?¿­bÖvF¼?¤/&ü˜¢´?®!¾¦ÀB?ì‡Ë>
%"?»HðË?±ª'b…—?²ã-Ø4¨ ?ÎeýtXá?±ëÜò!U?ä\dÅ7‹?¶¬8N­æN?À(oÓ­0ð?¨‹çØš?ÀTñtøÒõ?±ùîâ½ A?êw'õý?¶}{GêH¸?§9ȌÊôb?ž±iI#h)3FGL J1207.6-2232@r¸_.Q@C›ãø¶À9´ýµ¢äœÀ;Œ27Š±¿ád"†Ò@ñ3¼Æ@™@ ¦n¿â¦-QØöã¿éYA}h©¿éÜ ï'¯`¿ÛÉÀ¤õAGNbcu?ïEʤX õ?•ž$ºK?såý±?sJ³«q«?'M,K5+?"ae–U$?ï¤Ý³]oT?‹a®Á¦©œ?wc¤Eþù?'ýçé.ˆû?v-'ÈVF?z³>Å".?íÃÁ|¨¡Y?œs˜b€?—MÕqCcñ?‹÷"Q'?¨ý|Ô8‹?•QJ–F/?î«aæԖ\?˜…€]zg?fÿÍÅ
¸Ã?h¾3(‹Àá?£Ùä¶e¾°?˜ó3ê}ò3FGL J1208.2-7810c@rÊhŸÆÚEÀ.ùûg¿,À:7jÒñ²À; Ôký¿ó˜Õ¿9¼9@1<6½|@*A`y£¿èþv§kF¿ãOL÷¿ØuEWHw¿à©9c'»HAGNbcu ?ïï9ÚÈ©j?e"§¦¦[T?'¸òP¬Â?0Ïï"l?^•,$—«w?dS›¿¢'?ï¬÷`d?‡ÛÞzÃ¥?^¥¬øf®?k_+ÇÁ\?€írvÇó&?"T² cîg?îËñ[^)¿?ˆõwø4Èø?…ý:Û³K(?s4ð\*ù›?›ƒ7&a"¼?"Yn>¤w?ïv×b:?PyT(Vì?%àQâS?&©£›Zš?0Ñq´á?=ˆb©3FGL J1208.7+5442@`úMÓØ@N«"ßöu=À8rS±À;ÃÉfæ¾æ?çĝúZ\@{´+k>@X˜ÀUÆ¿äúÛùî÷x¿æá^‡IàÊ¿ç^Çζ0ÿ¿ïÿâóÍ3AGNfsrq?ïúQ,˜›?C+WdÓá?7Û×+õ?3o¦¸?7ušÄ:U?;¬®F¿ƒ›?ïҚc(QË?{!ò–ŒÄ¶?e››²xä?qã8KÁ¸?gÊÈû¼î?nìqš6â?îówπ?þd8Gœ†?'KÉSϏ¥?…g4µAæ?EF‹6€_?…t0¿1·?ïêœ)»û?pC$ÑØwÁ?G¶gg·Ã±?VÎdÑ¿ç?`ÉüVc?l5GÃ^«x3FGL J1209.1-5224@r†o€Uûµ@#܅_û¾'À9ùS‰XÀ;Œ¿Ígý¿öGþ3¢ï@
PëTø@Òc`¢'!¿éË"'È¿ç‰N'«?´¿Ý9iMM¿äø"PŒàNOTHERspp?)™€ ?Š3}ˆá?UL©n€‡?X0wÎúéÀ?…1 kÏÆñ?‰J,X ?ïkÁŸ(>@?˜¤þŒóî?eÇÞçJ{?k321oRe?Çæ>6?—¢uþ¼¨?îwf—Àb?"_ù>ëÝ?‹…:kck°?yR´J9±l?¡¨Gé&.ø?þăRå?ïY}'{á?†kÞOißF?(.º­G•†?-ÆMD1n?"Ÿý›BÔë?†LV[kö3FGL J1209.4+4119@bñàm"@RXfÀ(yœÀ:×YîˆßÀ;ÖEßÞ"¿÷ÁèW´›@SxW)²?ÿ2Àœ'È¿èѸ®Õ"¿á
+¥Rèä¿Ã7DԊB¿ãÏK4åCAGNbll?ïý™ä¿7?2ö"ë‡r>??/˞"K?Ÿ78oþá?)ÎéÎ=?Ê?,ýáÉ,¨A?ïÒ׸ZE¡?yF4%=C?`Éåë…Q?h64#ŠJ?l_8¿ÎÚt?rë$Ìßÿ?òø?w³k+­0"?qvõۑ³æ?p	¥>÷ߑ?}{êò®?n]ŒÖ|¼?ïꍎøYé?b¸;f-Ë>ôS(´•¹>ýd3—wl?eIʶ<ë~?b­3ˆj÷3FGL J1209.8+1810@oºèÀHZ@S9Y_í¦aÀ9gšA_EáÀ;¬ìµ `]?Ô¾t~
@ÐXAŠŽå@a>ÀZ"¶¿ÝF\ë¾T¿å¡•¹1±Ë¿çmP@Ê¿ãyU­lÆcAGNfsrq?ïóü攋'?X¾' {­?MÑüÚí'?Ug›z?B:hÓ¶ó?D4°×¾ž€?ïÖ^¦½Ç?vj%¾ã˜?]+dUHV?d$Üd0™ß?k3.ž'?q:&ÉþwŽ?ï ý{?ˆ£ŽµÆ?‡e†=!¼—?:|Ã+:?K=@lr?|äôŸ˜ÑÞ?ïßYÑ×Ì?p™íz®¿u?9š¾Í'?A!ûFÁÊQ?mƒ:Ñ#'º?p+†&vi3FGL J1212.2-6251@r§µŸôým¿Ôl(€/mßÀ7ʇJâ|aÀ9Äcôœ¯?ÀùÉ«ÁJŸ@Þao@ç v3¿àU¬9¯N7¿çF& 'Ó.¿é8¡Nè¿ãœ€w_OTHERspp?Ÿ:D5†äŠ?¢/à>ÎY?ϳN'ªB?Ï=ªwü±º?çf
¯^K?Ð+<âά?ăĸüO?Ê¡»4Fmg?³½¨×±â?»Èä~?èg‡³Ûžð?Αqà€¡?¸¬&ù<WB?¢[iówþ›?Ó-ËÒÎlè?·kwÑ<NÕ?ãS•7q>¤?¶ž[UW©?Ãõæã!§Ï?ÁSzke…h?"öG]>^?"Ɔ¶æ)?ê®­)ë?Á¯R]q¥3FGL J1212.6+5135@aÍ߆ã´@PM`#UÀ:'tVéñ¡À<ù7Žâ†¿¨n<OÕä@Å´'Œ¶@‡gÿ˜§¿è–'þõ¿¿Ú€]Q®5¿æÍNî-MI¿ã:©xx¦tAGNbll?ï˙{ÉR?"rN'Õ›W?v'͘²¹ ?"-ëeª{?P-Ò
äÅ?L5xÖ,½·?ï¯5†ìq¹?'s¥}.ˆ7?qº",÷©?súTľ"=?vª¸tš+Š?yƒVÐzøv?šf?‹¿=ͦ–?)g¥iñ?…ŠìÖd?‹ï5´TÑ?y[›zW÷?ïHýS?ƒEÛî?tø®|'Ý?p>UV¤n?ƒei]áí?}¼:é'3FGL J1213.1-2619@rE̟¶M@Aád ;ëÀ:1û9ÈÀ;¢þ‡Yûõ¿ì‹›óÄ{@`•™¯¾õ?þ.Ԟþ2u¿ÞµÁ"I«ñ¿ê¢%ùR«¿Ò‡¥; ?‡ÜèñÜAGNbll?ïóT
,å›?]xmaŒG·?úSKH?&'"cÌVa?WÈD?[Íd¥ˆô?ïË@<º'?~æ€ÖoÐ?d¿Cxžœƒ?i¢õŽå¼Ø?p@9Óhœ?ww]¹kKð?ïv¡++?‡ªŠé¾[2?ƒ§—éüÇ?wïrmÃ
Ã?"=`M*|>?'ÿlHê^?ïĆBÔÓ%?t8§î>ï]I¦>ÿ"ðW9?}­/ñ	ìA?t{†ì43FGL J1213.7+1306@pί€Uûµ@R[¢Àh¡À9¦¦J'RÀ;ÁžÊ[…?îâä]&£@r°¹Æµ±@([À6ã¿ãœýd¢Êx¿åݙíÁ'í¿ëÉV~D‡¿ï÷c"ã©AGNfsrq?èÔ?Ã/=îZ;?ÃøhÚ
|?¼Üf8Òê?³—Êw«Äê?³® D'Ö?×÷Ž,¼?Ð	úûõýî?á@©ÚÀ®?ϝz¤5—?¶xµLŠ?¹7CÈ4ƒ?é­IáçUÞ?®¥ÊÜ]T?½ xÿœ£®?¥!Þxõ'ú?µu7ñ(­g?¡RIå‡?Äñ|"¤÷<?³4¸Çp?él¸ê­N‹?·õ­ueØ?¥n—:i?¢ú1K‰7Ú3FGL J1214.0-6236@rªI`0Â@¿ª×'?á
À7Öå•ñnmÀ9Õܨ#$?÷Nu»€Ê@>:\È-?þ¿Ü™žw$¿º}bVa`˜¿ãÜ[ýVØ¿å%±Ím¿ézØC""OTHERspp?h›H'ÏúO?e£¢ç¿Y?¾ÃÐFµZ?Á¥îý£+)?ìê¯"Æ?ÁÍ77ô#ž?|÷w)u'?ˆsXj«õ?¾ñ½;–ª§?¶ ä͕"Ë?ëçÙjn×À?·`è™}ÃÅ?¦ÛÕZ}¾?–Ó¼±R?Í~~îX?²m'ΙIÛ?çP#)7<Ž?²áš5H³æ?ªm­[²´/?¦íEA'+?»dƒ›æW?ª|EéŸ?êøؙÑWò?µÃkŠú3FGL J1215.0+5002@a,ô!-w@Pƒ¾`"‡À9þ1Ýȝ"À;ÔÇýZ3R?Ô¶G5"ØS@RÙþ
·y?þ¶
 r~?ïIJá$É¿çoO ž¿ÁTªYãÔ¯¿åѱ'­AGNbll?ï½;̂t?'ÏÔ!ó²š?J)råø»ï?K—@?~ëbçµ?æ†Š¢l?ïsv®½á‰?Œª'ðê?M´ã%íÈ?_k¥$?ÔŸma°?'ê'ðö$?î݆3`>õ?Ä+RLÆ?ˆ	HÙÀ%¸?{Üdþ	?˜J•'‡?†XÀÖ;è!?îl%`ä?¦*ٙW?†Ð֝ئç?‰úPŸd‹G?©å{–?¤>@µ…3FGL J1215.1+1658@pW"_ôö@S4z?̞ªÀ9´`ÎvñÀ;Àh‹Ô¡?èRßúÅ:@Gt.©6@‡¼Ÿ®·¿Ð1Ƽ›¿å¹6²Ää¿é÷ÏM
WŠ¿äœGãˆ?AGNfsrq?îÕLyÈ7€?±,AÞÑ?¡ÝÃi…d?°ñZ/Ÿ.?juª0*N?m«ýÝZMÆ?îöÕo¡pØ?¢MgÀž=?T¯îò@9?–ßä·b'ˆ?Ð¢ߤº?™ º‹†?î>‡5
?˜e7ŽØ3>?»ÖA̒?'ÌÞ»²D»?šsH/בÒ?‡ˆx Àþ?ê7>Y¶è?µ¯†K&?¿Ú¦¸D¯?´F¡¶Éi?¬ÖÌô\õ?¦Þl;»Ÿ93FGL J1217.8+3007@g›îàóË>@TƒDàá6À7i1"·ºíÀ:®•­¤é?å^·üŽ¹õ@Qˆ®d×Æ?ÿ—v~·k¿àÉø՜޿àDOÌಢ¿ßÃ`uiA@¿áùùšzAGNbll?ïÙmµ¯þ?­ ?‰³ˆ?3Ríêˆ?5ƒsJÊù?röIXyý?­¢7ëͅu?ïÁ¥N¤úX?ˆ™2ؾ?Õ?bÅÔ¸÷?jÝ»'¡À"?võÃ&X?‡s[+`?î¼yÛ[?˜PK^gW·?~þ6
ºc¸?Àê4Ý=%? X›ˆ÷l?•'P€°Ü‹?ïC©aô¸?•âÑOÀŒƒ?[Rþ£~ê$?fe§z?œbZé‰z<?•œèÏÛË=3FGL J1218.0-0029@qÖÿâ£Ï@N¢ŸÒ˜¿À9|Æ@Á'/À;sþ¨+¡?àÁ Á"—@··M^­Š@]a#Ü¿äóa£ý‡¿åjÊ!)xþ¿êGDŒ™Mf¿ÑºO­ÎkAGNbll?ï鈆
ô?h±©y]?_"f|f­Ã?c·sxğ¢?K™ÞºÔÿ?N"ZÎZ£?ïÌWÂ\%?~ÎÝà®mû?i<—¿ûpe?sWÄ©'E©?jk¥ãøj(?p%ÎËÕ¨?ï=¦ƒ÷8:?†T[IYÐF?ƒÔÓnžb"?€
'rdÓ
?ŒÁ‹""Žæ?{ŵðvÜ?ïC‰›¿?ŽÏ췄À`?jõì3•(¸?q¯ùqà4?"@'FzC?X>2èÁ%3FGL J1218.4-0121@qà|`Ÿ@N5æ`ɊÀ9hq¡›À;`qå©é?Þ0$ðˆ@RìéLà-@Á?zê,¿Úà'yõíá¿áVzšÖ»¿æùïã&¿Ö·µœb)sAGNbll?ïe´ø"]Ž?°™wÝá¶&?ˆò ø°?°–ìŒj?frsᜰ?iä¨9?ïa4øKÖ?ñ¹Uïf?|áÄ«)¦?‰69ü÷E?{m Ø°o?}
ËóWÖÂ?í'\yÁoã?¡'xYØ/e?¡aêIEѤ?"Î*Söµ?¦xN£0#?–aê?í((k3­®?¤bìyøÉ?—$Ž_Ép?•F]ÃÁ(ð?°õ™p6‡?£Eä¥&3FGL J1218.5+6912@_Ïÿ`Ï‰@GÑN¿ÓÀÀ:O…¯
À<îøp¿†¿e»_p_¯Ú@¡P&l@&îÿ|¢h¿ê³~ÁT¿çÚ:Þo®Ü¿ïª¦!ÅÖ¿ïí7©¬–AGNbcu?ï)ö{ ?»50¶¿Ñ?še·ÄW?»6Í⏯~?7Içñéã?C¢Y_å88?îž_¡Ù?¤×k_ïúû?œÍ‹ÊOq?Ÿý—Oá\?ŽÞ!"Üêí?'¼%Êɍ2?îe3‹û£?–´Æ4¢	?$mO'k?'Abòœì?–Xõ!1	%?Šúk§DÉ?ësÛ_~Ä]?·'#±LnP?¼"zd"•ò?¶W':·ES?Ÿ6ª}Ù›?š!]™Í,3FGL J1218.8-4827@r•øŸƒ¾f@,•"d~À9—æuë>¨À;…ª8MNg?ÃA¡b2Fœ@ÅUmðžc@°zÿzŸ¿á»Â/Ý4Æ¿âR1ÙR¿ã-1ò&µ¿ïäšZAGNbcu?è 35ó5(?ÄPÑò½Ž?ă»è¦…¼?ÀZÆ+Áhc?µöîKO?³‡6;HÆÔ?ê>(8?Á_%Â;«?µ]ån¯AE?¯î¢u‡¹?¹à)O(?ºXÊÐjèº?éü¾ó§1?®byx1	`?¿ã'ô¸Ëþ?¨LyÂÌÊ?°6àn2r?™:Íõ?é°¼õe}?­ÒA¦I·j?³VWP'*?¥¨?²þ±?¿#Á?D¬ò?¤Ì'˜ñµ[3FGL J1219.7-0314@qù€#¦Î@MWý`OÀ9ÆÀâ³¾ßÀ;–ÿ³©æ?䓒T3'†@Á!ý*ãƒ@Ÿ§Ð"¿Öyw8':¿ÞU#ÁXØè¿à'Ž:ô¿âߙ
AGNbll?ïâΰõM?ž}^"ö?ˆØÈÖ¹ho?'¹÷Y§>?®ƒ}	D~?•Ø'ºoÑ?îa¦PÁò?©º,ìÀD%?¡¢iÌ3ð?¥y0¨Î½?†bOt?'.å¶?mA?íñ"Õ¤ÃÛ?š) ž'¾]?™œÏ'"€¯?‰½=Ê{­?¤Jäjö?'Éq"¼e/?éÊﮧ|?®•øÇè;?·sŽ–»ÅÈ?ª‡ÖV.Sq?º4øƒÎþY?¤V"çufQ3FGL J1220.2+3434@d^Õ•:@Sÿí ‹]À9à5"FK>À;éC¡É¿êÕõ7zÄ@`<O´X@oÿl\J¿áò¼:ƒ^š¿áËcÁ¤\¿äŠÝcÈÒA¿æàBÙL´AGNbll?ïšU¬Ão?‰½ºm*?s…øßQVù?sæÁnà"?OƒJLñ‡?…t®Hö|?ï}ÄN üz?™ÙÁC7T?u&=&ö‡œ?€±mø/Ð?…ûÍÄEÄ?–r-Pp?î˜?"}`»?"§ÛQ«š?Ž:%†Ukh?'†z'mb£?ÚúÍ)3
?0n¬­¿?ïw~ÃsÐ?‹F+ó@J·?mlÇÀcŸG?pëV,ü¶e?ŠÅ3$7?ˆtÖC`šS3FGL J1220.2+7105@_¢ïÝëÙ@Fè|à%o%À9Œõ#-+²À<|Ñâ¶C?Ò@XXå@ {KÆÓ@²¾ aŸW¿äII0[Ï¿åÁc"&¿ê"x×Æꤿè[ki;¥AGNfsrq?ïø†Ä—t,?IØ­ŽFª?A3ëì¿Ó?EH
T`?9bjÞð(?7°¨g})?ïÆÙxJÇ?z«
Æدï?liMœ^¶™?oò*¼!é(?l½:œ"k?qM'«d?ïW'F9o?†&'QÂ?€ö\#ª³?XÎZÁ÷l?‰?Òmšù±?zc%"õ?ïÔqZ%?wLdLÞX…?T«8²~žñ?U¬<®·«?pœ¦Ê³EG?vGxRÒ\Á3FGL J1221.3+3010@gKØ't@T¯ &5À7É©f–7À:ˆ'–9?ٌ0¡Ð@Zys3~?úèÀž@G?¦cMû¿Û(ó/sû¿ÎŸ5åÀ¿Ñk…ÎÐK÷AGNbll?ïÒíÆ7ü?~ÿ
Ç`Þ0?@ÝÔ¨U?D¦¬'í?tmbt,œ?}±±Tˆ'—?ï¾Ñ"n…?Œ[|î–)·?cMÿâz?m@CtYY±?vð=׀t®?‹¶&§­È?çR¦¨Dý—?´*0§ò'À?¢kS8&õõ?˜&ÓFQ?ΐâL(?³âàŠHÑ?ëâÓñQ@?±mè½'??håp³¢˜Ì?qi³°{óŠ?Àwíd˜?±mËÖõû/3FGL J1221.4+2814@i5ÛߏG0@TÑî¿Ñ;ÇÀ7ÍÜcBÅwÀ;#Pg ¡?ëäb''k'@Fö¬o4@@Ñ£@Œb$¿Þ"yt51¿â'î÷øŒ¿àܽýôY{¿åXlR¹‹RAGNbll?ï՞­†}Ç?­Ä–®4©T?7
g¯M?5<ãõ˜b?s¿ÒÁψI?­Ç̔ºG?ï»ÒP
ßò?ˆ.F+Dº?fÚ\òü?o_ò`"Ø?v©©ñ.-§?†p6Kᓟ?ï7eÏԜ?‹zèµ%J?…HøM©?yÃJÊy‹Œ?';¡ò.?‡.Tš F?ï"xkE?––:ðÒ34?põÎï{?to}jÖ–?—°µkËt?•÷K°yd3FGL J1222.4+0414@q͞?»×²@P…IÿþRÀ8Fˆ'
YÀ;I_ND0±?õ±Óšt¦@ôDÖÙZ@Aâ:È'÷¿åk´¿˜dn¿ê–î¼ê4D¿ìíâtåì?¿ÝÌùˆA­tAGNfsrq?ïö¥‹IJ?\5*ê>?Gó6!U"?Q_G;šÛ?:í9u‹K?SŒÂè!Ä?ïÅ1ÂÛI1?}€o|¶"?j+FR)?p"|¸ã\?p\ï2RÉ?s`ëM`›?î›o+•EZ?—Ž¼º¥€?')Ò[~/?Š)ØD"VÐ?›hVúûÖ|?'ÞÙ
x?–?î–6Y†c‹?£¥ Çã'1?‹XöúâR?"ƒ{1¦Ý?ŸŒ¹Ì6š?¡ÒH–ùì3FGL J1222.7+8041@_rÞCí–@B,Ò?ÓT¦À9+ªëÑtÒÀ;Ç«ZŒ='?×ي)(H@áuÁ"I¬@HÿÚÁ,¿à½'i›ò¿æÔ/[¿áå(­b3¿ê¸ƒÑJ#ÔAGNbll?ïè>ÍXÈ4?d˜·ÐÐ?Pɶ9M?IƼ®p"?_pœ;¹_)?aÌáQi?ï66€2½?'±Œœ"?‹2È0âÀ¦?†©ÍP½©×?‡?—ÂyP?†zBÄñÉ?Äu'1?–D!úh?")"À\?‹èÒ8ω'?–ê`¸ù²?Œ,Ço†ï?qº¼ ?šj|b)?‰2V=Û?ƒBjÇŽ³?Fº	~l?–ÅIDeD3FGL J1223.3-3028@r|˟ÛÒú@@‰`fr%À:vŽŒ]"À;¼ól|*?Âv¥´ì@
¼Œã¨±?þ/ƒáK‰ì¿ãšOˆ¿åüqЧͺ¿Ü
«±Ò©¿ÉW̵AGNbcu?ïÙ r\qu?xíJ-ð²£?2´.Áæqœ?2¹u†,‹?rƒå¨Þi?xqEÃm¿w?ï¸ÐÛo<W?€
Yé¼O?müñyË7ã?o¹=»é?t™‹|8@?w¨oé°ß™?ï_;¼I[?‰˜¾cÒb'?ýΘÑHÉ?rWÃ)- ?–µ1</þ?"6'"]q?ïAÏ&qí
?Žµ^7ÍÁ?P†öwµ?YL2Ti~€?–½«ÊIƒ,?Ž;
%,å 3FGL J1224.5+4957@`¼ÿÚ@S@P¥é`êMÀ:=އà4À;á¼é)ú¥¿Â¥ô*]³@L¤sgUÐ@´¶ŸcÝö¿âµý¨ëNÌ¿ë'Éùkø¿Ó7"E5­ü¿ëôHÖAGNfsrq?ï슺i"œ?fuƒ¡‹C1?AhE
Ü[â?@;1¸ú?^6h§ˆšx?d]öù£?ï¤âU?žÿ?"¿ã×À?u¦ûäkÃÿ?yÒmlw?wçÙ{ļø?yüÄ®gß"?îÃýlì?~¨hFL¸?‹Xº?€¥Þl:q?˜º•&í61?‰×Á¾{E\?ïYÿWÉ˚?ŠÔ w£Õ?hè@NÖΘ?j\'¾ìŠj?'£üë²â?ˆN±:vŽ3FGL J1224.5+2436@m@ôŸM¡@Tܸ¿ÏŽHÀ9†_:øúRÀ;ˆ›†Ù£?μÛÙì+H@𪮔Óa?þ0é
ìî¿éŒT¼ð¶·¿Õ0yשÁý¿ÔûòÇ)¿ãπل@AAGNbll?ïÊ¢JÅê?ª¯Šù?L—^0ëµ ?Mú}t·È?wï1"Ç?ª²Õ+-?ïk_ØÀ%?•Eb¦êhè?zŒ âmÛ?$pQ)?‡áÿ¿‡¿?".v'Z?ï)ɇ¬7n?Šßӆ)?	¥4?v+KÕ$	í?'B7õ÷æ?‡óPÞÝ?îϘyêj?'|¤â?Z´,ÇäR?x
}ÌOÒ
?pRÚ^ÀŒ?˜ß¦ü¬õ3FGL J1224.6+4332@anýæOU@R-‹àôÀ9´Rb£cGÀ;ÿžÁ÷†µ¿àºñQ!ÁØ@­á­.¡Ô@]  Ö¿æh¨µì6¿è õ(¿Ž¿æW|ûBð¿ïÿ⾦™\AGNbll?ïìêî?˜ÒfZ»?[š©ïpœ?˜nUDv?HNPugn ?Rcbóì?ï2ÿ`5?˜ž…—vÇ?‰Þ£}‰$¿?>uÕÓÒ?‰a"u5Ӈ?Ž¤çò¸ú?ï:Žˆ"H*?‰»Þ¥r?†/jù%¸ü?{‰%Yíœ?‹,òþH<¡?"TœË§ß?îѽA‰Ng?üLڑˆ?"èŠ
6¾?–¨DL. x?'àHDÈüP?q…œÛç3FGL J1224.6-8312@ráoŸËÀ4a¦¹Ù«À9zeÜÓ«
À;{ ù	kº?¹3ݕ+}@#ÏÃøõ@Ž_?«'"¿ä‰'å´g¿êj\´Ù2ƒ¿ãü¶Ôâm¿í|3FUAGNbcu?îçNýJä? ~úþ&d?…²ß)Ƽ¹?ŸãgZÈ?˜<°ÇÓE?šI'ZLÂ?îqåaÏJd?¨ê%©AØ8?ŒjjRSX?Ž½2zäŸü?¡ÇvÄð?¤B¤€UÎk?ëí҂JˆÜ?¦ú^¹ 4 ?±YÚFÖ?ž¾oÉ?®o#ºËLŒ?™ÎécUG?ë®ûHŠóˆ?¦¨ß^^Ùí?é²áÞ¸á?p)EݗS?¾Šï_lŒ±?¦I °½¶3FGL J1224.9+2122@oáç_ö	Ý@TjV ŘÀ5û‰SÑ8lÀ:e~ƒ"×?ù»]¹™";@#šŽSz@ñcá¦Î‹¿á"ìÂû+Ÿ¿åOA
çIP¿äÔ]X†åô¿çH%p|ê·AGNFSRQ?﹍`;Æ?ƒÔÂD|·?_)0[&a?a01z?{oË­–Ó?'ëGyi?ïÔ¿µ?ßÀ{ª'`?[ܦhª¬?f>½å;n?møíÆ*õ¥?|Hs>Þä\?ìÀÝ#…
?¨¤½Tq?›iª£RGú?"Y¥·Âkß?³%VnEœ?£X1fÅÉL?ïÿh¾?-;ØJø>ŠçAE0'>´1ϼíß3?àt‹ºº}?-:çÆ8k¼3FGL J1225.7-7314@rÐÛ«–òÀ$íG¾Ûr'À9á¢!þW‰À;s`c'¿ò©0
3à'@>}[ËWØ@y¬ÿ§ël?çöE€‰q¿ìãrÜÁ¿Àvö%$–|¿çã•&ÔfZAGNbcu?íM*—Á?¾£ö
Q5?m©éˆD•ä?xÂýô"ð?¶xG^ÿÓF?½ªQ;•ƒ=?î¢c?FoÈ?¯ÔLè'?pÝ­iBC?z…Gñ'—?£¾^v[C?®"Ð…œ/?ì'5'÷?£ïüKÒÕh?"ÆIŠ†ƒ?ŠŽ2Á?´/LÅpΧ? cq}!g:?î/!ø~ŠK?¡¨–ãëÛ?-ŒqŽ@ÜT?:nzs•Î?¬ðT‰g?¡©,~¹Ôƒ3FGL J1226.8+0638@qÝõ€í @Q,ڀ¶–À:ámmÁ¤À;·ÉjA½:¿ÔôU–¤6@
‹w+/®™?ù>ÎÇÏ¿í··pˆíê¿ßø…Š…Q?ʦ`;ÿàu¿ÕS{ìÏ:AGNbll?ïú·hUô
?OAE§sÌy?#cŸ`ço?%€…¸àK?@Iz€W N?N5v4 4W?ï¼_Í"ù?"žØë
ê?k¢dæb¸?sŸ©Z*Ã?sÿ
ÁÊQö?}É¡WµÜ'?ïë~÷P?ˆ\
_O?†jåÐsÛ?€÷H‰-þ?'
8Ü!?¿–]VÈ?ïI‹–í??'"TÏË?7í~ۃӽ?F"±<XÝ1?–n×&ïÈØ?'Š¸Ñr¯²3FGL J1226.9-1329@r]®@…+N@Hxwò
ÏÀ9.x,a‡ÚÀ;R½¿Ïæ?îƒÝy\&5@KŠó8œT?ÿ¹V  žñ¿ïþÞY‰€"?ïèÏ;*è%¿á"30¦]¿åY¬µç´AGNbll?ïˆÃÄ{$?‰ˆó÷Rx³?ƒì'Ä"r?"þÒç~y?tx•¥e$?sÝî«K\s?çDmK©c?Íd·R{Ž?Î"|JVq?ÌIvÕ¨?¦ß/:?¨îd¤…?퇗ýæÕ}? "ø9eÏ?¥mÃ	'I?—¢Øå<~?¢z^‰Þ?"9œ5P?ۋJúíÃ?Ènç/ƒ?áEgùx?Ê*A>?žžo¿'#?¢à§é"Ò)3FGL J1227.9-4854@r¯CÀ~à±@+"É¡Ÿ!™À7蠖ãÜ´À;ϹWf?ø‡¤Ò1æ'@Džïnã8@–5¶ñ¿âZˆKµØa¿äP¡KÐÊ¿çü?^Ã8¿êßÿ_PSRpsr?åΙóa?ÇcÅúj"A?̎hײE?ÃLbZÖ?¸rc*µ"?¹âhhˆÃ?ЫL
:h?Ë®,6=_?á±ñњ?Îds àç?Çᣢ"#?Ä«tì‡IJ?å€Ð'ÿÖT?³|y	b‹d?ÊM¡/õî?°€Öx|Ց?¿^91¡a…?£»:'2?É1Tà?Ü?³fŠ7¦c?ã`šÝÚÜ?½MZ&­ê?ÉL?«At¹?¶ªhšî'Ò3FGL J1228.7+4857@`™¥ 8L@Pî‹î²ÑÀ9èûŒ3€À;©ÏŽH,¿¿Â–Lwg@á©Ë•ë@ë€z8Ö¿äVˆ: ¸1¿äS‰ëY]r¿í94?*jë?Ì9¿ãǪAGNfsrq?ïçsÖk³>?hØ 'ï?QÉB'Žd?RϺáˆ?_O–«?dp6(~ض?ïÔÉlõæÕ?y?	xM¶ë?a:zŠmj?jgØZwÂ?iüŽ¾X?p)¢ú,¼?ïB!ãMñ…?†C'ÆOV"?«Üu"Š?y<.Sv.W?Ëª¶ÿÿ?]œG?ïÞJ=dûW?r)Óë†ÉÈ?1]»I‡÷Ÿ?C›±¤¼‹f?oŠ1Ó©Š?qé2zþ½y3FGL J1229.1+0202@r¨@[9â@Pr@#Ü~À6nç=À:Üš\78?ÿ£"¦%@!ñ@­DFV@Zâ"o¿å±*SrÁ¿é8÷(JL¿êjÏÃ2€l¿êw({Y\AGNFSRQ?ïâïøÑÕá?u/À'/‡T?gš˜>L¼?tsEŸ4M?H²W¯Bþ?P¥{O?ïܐ¼¼²?v»uDŽÕ?]B•åè'?h([íFA?dçÆøPYn?l^~'È?ìÉr¼ŽG?¦–Ì+…È?¯y€.˜V?¢
€­D2?£ÐŸTƒ?™ãëï
0€?ïþDHÞÅ?Gæ
2l>ë¨øÜÍ×)?'UÉ¥±c?*â'ÙT?G3ô5åúÒ3FGL J1229.8-5305@rºm ‹]@#H>¿ÙI]À:;zç&ë&À;Žã©8?°V)bßO@5Ãm}†é@,àŸ©¿èohÚ£¾Ð¿ècVX.ª¿ÑÙ9x'ÙË¿à`Á`¥AGNbcu?ïç˜Ñ+¦â?p"–Ĝ0?#ڟÐÔ<ò?%X–üsîp?g)"×KØõ?pc/ê‹}c?">îj?¨Æ'[ƒß?q˜GD?sqKßþHÛ?£AõÉP|?§ï	íÍò?îÐfýÒà?"çÉd{Å,?|
"éëV'?s,ŒAßÆ?žüŽ%ÊÎ]?'µå>ï?ïP©Oîdÿ?‡¸'ÚQkb?4qbq?¨Ö?=–©§gsà?•™xna{?‡kPÌ‰%3FGL J1230.3+2519@mF`¢G@U;{ îÙÀ9PY´§<À;Ÿ"ËÜâÅ?é¬^U©]e@:ä1Bm8@âàK¯¬¿Ðad¸«'¿å9ýgIeO¿ã߃ÍnL¿æ-b†Ì§AGNbll?ïðY#	7¿?xMÙ_šÉÿ?@ÖÈBc¥?<âˆ2Moì?VâŬS~?xß»»;´?ïƒÆ\°ƒ ?'²ÞÌÙ?wçÙ`
úÐ?Y™˜ä"?ƒ|#Ø:Q?Iâïؔ?îÎ-+¹bè?'TƁ$?¿Te
d?"ù+OD~?—Z°VLÔ?ŒЄÿÙJ?îtæü² ?Ÿ¬ÛoÔP?•5·Ï•;_?ŽÉ1Í*‡Y?œ-hš&à?šÎÊ+?3FGL J1230.9+1224@q½lºËC@R ÂÀ®À8ô>A"/À;c‰ì}l<?½óg¥<@ôÖÂ@R`0lY¿Òð‰«öú"¿á/¬i0Š¿ßÝí3¨,¿éÅN>b¢AGNrdg?íÒ²HBÜM?©+•ÐFÙI?¥v\}à?¢œ ¥×2Ð?šˆÊòëz›?.É¡®¬?î'©€
s?¯µq¹ŒÜŒ?œÊy-??¢µÇ¯«µL?ž@d'¿@,?¨
G]ã¾µ?êÔâ¢ekë?®87Åòµ?¹%§«Vï?§ø€qԑ»?°3CA}±—?š'óãg''?ê¯a¸wJÅ?²b`é-]?°á¢wU?¸?§Ÿÿé3ȧ?¹£OÄðj?ª»åPÏӛ3FGL J1231.2-1411@rxž?»×²@H1ÀY!À6ÿcëaãJÀ:á\·ûe@	dŠ÷t@DETH?ûšÞ˜–?¯ñO8!"Š¿Ù|µ^C¿ãV^´ó¿í«Kô±S†PSRPSR?NE"¾we?N.ê÷ÐFl?ïñ)šœQï?YïûVÏÃ?MÐ@ÜÔ?O(X۟›Ï?uZúCÒ@P?¡U¢Í¥Îo?ïU[/j¼??¬2$«æŠ#?û·gÐ?£ý"[ÄY?­eI~±*Á?¡:?ÿS¬?ìw˜óÔ7?£ƒÌǑ5è?«)üò'Ã?"VE_=åt?.~÷nMd?30ç×µ†?ïØ۟ɼ?teB¡þv?rž8_Ͷà?s·fî#µ¬3FGL J1231.5+6414@_ qÁ
{ê@J`»oÀ: 'oÿl\À<PœÐ…¿?×Ì°áù@2ugMA?ÿwß	»@¿¥' x'Û¿×PÈfØôp¿ç;Cɔš=?Æ4U-j,«AGNbll?ïŒbÜé?±UyN£ãL?›ñïS…?±KEŠ,?aä%zۇ?gEªv"}?ïª
éº]?‹j6PÍ]?wèمŠSY?…7¼ZÉç?s1f}y?x¦
Õ|½?íìg˜. ?žìP?(??£œ_˜pí?ššiÀÖÁ?›D3Üõ?ˆjCv¯˜?ïwÇ;tNØ?4å÷x,?wü3"!?…ªÞIWà?†—ä9?†Ìzض^°3FGL J1231.7+2847@gÙü?O@UV™¦5À82~5ÅÀ;
3Ï:eW?ã쏪yÞ
@C¨×¥ý?ÿ-À"!¿ÞÁ¼š½ ¿àÞúvÔ¿Ý7ÁÉu¿ßÃt|9óAGNbll?ïúök~Q?B˜Õ¡Ø?)Á	'¯<?&³3˳Ø?AsãíZì²?>ºd¸Ë¬"?ïÃÌ`d q?"¾ÜáôêÜ?ddæîÀd?qý¬&'?sç\ĸfÃ?ñYš/kì?ïr؞y?™;ðwþ?vp?o¯Øý?rû'®'?ˆAê ‰¯×?yËg"cè?ïbSÍXŠ?‹KÞå­Õ?WœÁàm
?\´µ®¹?';º6õ(?Š˜…6…>R3FGL J1231.8+1421@q¤˜ˆv\@St÷íÀ:,÷öFBÚÀ;¼ùS="¶ÀŽ_¡¦-|@4Ö8±Li@…=ÀªÕ¿âqõ!¿ä+t¡´è¿ÜŒBX•¿äҏ™AGNbll?ï­"Ä>]w?èëHŠ%H?Fºô¨'›?KÆú¤kd²?ƒUsA?@×Äx&G?ïÉ-iââ?ƒUXwj?a Ëœ+?k¶"+?rÜjz¨Á?€áø£ÂYL?îɍW•J¡?'èÛ5ƒü?"–7U£?tW¸««ô+?œ¿	ñ–é?srw'ð"?ïНåÆ?x\pc£?
EÍx½—?$iYgZ?w|ò'õ?wÝpžñˆ3FGL J1233.7-0145@r]cÿï9@Nf­ _À9úö«ÃhÀ;{µò•´?ÙÝW^‹§@üsƒôl@ÅhpM›¿åÚ¯/û<Ä¿ã<A"<ɿ㖭gÆ|•¿ÒÏç&×AGNbll?ì÷øZæ´[?¸1Œ"?7Ñõ{wt?‰Ò0OF?´YBêî>?·—°(¸Ø?ï
Åmo?©»WÝ?¦4?'RšïqÊ'? ð{¹	³@?‰÷ïÁÙ?˜‡Dp9Ê´?먞>¿?§²‡çÙ,?¥÷HB¼×?"áÉG¿?·¿kœ¬¦?£>Ü=ݜù?ëE0¾_‰•?²`A>‹ND?¥º½Ã"bx?§è'êt˜?ºù+:?­¶binœ[3FGL J1233.9-5736@rÉf?šIÃ@½ËCòžÀ8ÊÅ­ÚÜÀ; Îô©‹¿ðØOÒ¦*¢@Aˆ£¨U@Pèß|ý­¿æ¢.§n¡¿ÞèžÞä
¿âÿÉjä¿ÝE?IR@AGNbcu?íSM-¶?±éÒÇÀî?z}ñ¬YÏ?s×a_g'?³½·wŠN—?±nt–Uèu?ì…$Ñw?À•J¾Áð	?~ìwìÖý.?…gϐÚbÕ?¹è'©Ìs?Àúp´?êO¥ÌÂ*<?­+©ˆéG?ªJ"Í"?"a]Ì?À=Ö+ÄÅ?§ç3nÕfz?í.¹#,¾?¥â AUPÕ?Xb̋•cV?_"–çË&ø?·ÿ¸DŠ?¥Ìä‰!yÜ3FGL J1236.6+3901@a&°)(@Sm~ßÙïËÀ:~1«s¶±À<
M`Ûã?Ä¡‹Sc\ú@0"[—*@ï·¿ttœ¿îFK­—A>¿È:́ʿã—e{ž¡¿Ø2Ÿ,´¯AGNbll?ïÕà 
ïš?‰Ë5τã?]ð˜2)3û?mújÃQ?k'ÛûËÆ?‡%s5ù?ïžÖ­œé ?"Sª?˜°?qÇÀ|¸þ?z	Õ|bŠG?~Ìèµov~?'ht)WB™?î|‰5Ç'?•k!ÚB‹]?"— ä†à?‰§ñ\Xþ?œ×W¦9‡?ã9w€W}?ïw‡MÒ&ˆ?‡@…¯äÏ?€Äò"Ñ^‹?X¿?•?Y9÷¤þü?|ü¡­ÎÄT3FGL J1237.9+6258@_b^AÔ¶¦@K
q VL=À:Ƽj~ùÛÀ<+Š«ÀË¿È;Ki¤£'@% ¢!}~?ýb
Cœ¸¿ìُ&_K{¿Ù¨L·"«¿Ön°Ëu›¿ÔlZÚàaAGNbll?ïä͝<?xQ=X§Í†?iaÇKô`?wÏó±¬6?-Ö'€Ð`?>Ó¤þšTP?è"É?X6CÚ(?|§wÈ}ÄE?ˆKž¼§7ò?x€"õ­¹?})h9ØÖ³?î¶^t	§¤?šêZ?œæW©®m?šæ,Ï@ƒk?ˆ›³ª9<Ï?sqmÝò×±?")T¡?'ãø?èÃ?X)ì¡^?_µ_9?…–]aN?' ZÈáÌ3FGL J1238.2-1958@r«f?šIÃ@EcêßÝJÉÀ9¾RsjZèÀ;´'¾ÙÅ?ÖÍ25K*@)ìþñb-@ÊÀYY¿éå-¤Òï¿á©ÉÆÍ¿Þãµ¼ºÛß¿ë¿öAGNbcu?í±,5¤˜b?°Jº]{!¯?°}¶åîÄJ?¯_Îǽœ?ŽvÎNJë?…í÷³¾×?îjP…OIê?¡†Z'Õ? 4•&¡r?›Œ|ۜX ?'LÅÓ£é?'¥|'°êÒ?ì÷×½©?£¨áÓ`5ç?«	Ñ\Á?šF€pâù?¥w†ÑsÝ?•dd'q…r?í>´¸§f? cçö̏g?¡ƒ4‹½©?"l9˜ƒ-e?ª'òøxî?™˜òè¤-3FGL J1238.3-4543@rÈÇ`|Aš@1cÀ™¸£À9Îä¦f&À;©:}ªP¿ï™£ÒO)@|b¤dùª@9Ê?©¹!¿í¿:ÓI?¢‹ºÖ!¬š¿à'n¦`ý¿åÔórFfAGNbcu?ïèdgéð?s EŠe?IýÓë]÷?K¦qýJ{?`ã&>"5?r~þt?dÙ?ï¤å·uµÞ?‰åGyª‹Î?h½ýX®d?tZ–g[ª?€—Ú¼\À?"ÈJ 2:Ý?ï8É÷02?Š+Ò$¡9µ?"oàó·?€uÖßÙ?â¡@<G?'ÜŒ—Ót?ﵧ­åŒ'?xƃà¾?HØ2í2Õ?NùØúÞzæ?'WÉÉ?x†V
R3FGL J1239.4+0727@rc}sÉ@QˆfxÀ9½â¯ åÀ;§†_*2¿ñŽÑú‰ @j«Yàq@.Bß·7¿éÓì$<0™¿á@­åßuú¿åì''GK¿ã¤	"AGNbcu?Hˆ^?uÌw•h?}ñ½`hU5?€®ÃÂÏ?Až[h¡Š?'ÛœVk¾î?ﴆɆ"%?'Ù¸t¬Wí?pyEMj?vÚ+|¹}?uCU¯hÙø?we°s©ž¯?îsbÍèÄ?š·¤Q¨,?–Y+×¾?ˆi;ksLC?£¬F½•‡ï?"I
ûéµh?ï[¸q#?‰Î¼
dy_?`×û
ØQ¤?bÎÊï›á?''iƒ1\?ˆŽÖ–¯U.3FGL J1239.5+0443@rs‰ :2+@PÚqÿ÷œ"À7'Œö(/À;¢!'—ô?ûuëæmˆ@ŒIõl~.@í*#•‹¿ágï¨nô¿å¥9¤¿æfâN3Œ¿êîÀmvƒžAGNfsrq?ï½$Ek/€?ƒXûksY?{2^ËÝÐ?'äÜ'>?Xíùú)½º?fuï۞$?ï۝¢ž<ä?u¨"À{C
?\ؔ!m'3?gyÞ¿ê=?eöQ\"?oko8]–L?íWTõK?¥=5!ÑT²?¯Mw\!?¡Ī¢ð?Ÿ:†©&Q?"˜DÚÍ<?ïîÇ«-±Î?l_4'U¶?-cÑd±]?G«_]	d?^Ä/x›?kvñN²U?3FGL J1241.6-1456@r¶a_Ìr@Gíù?ò^WÀ:C5'Ì÷À;Ækš'Í¥?â'AêÂ<a@º¿-§Ù?ÿYÊÿ˜&'¿îhŽa'&?žGь
v¿Ôyµ€¸Í¿ãé<¾5AGNbll?ïä:'Mx[?"(ûëX‰º?^¬èÈ1ÿ›?wk"?XÝôœÝIÊ?rÙV‡r?íðwÍQ3?ªԕ"!X?§Êáöë–%?§ZÍ·ƒî¼?'[Bhoñ?'Ì® É®ê?ï48Ä?ƒnÆê%?ƒÙ!¢‰'ç?v1
íPº?Öìq©€?xhxâS?ì™Åj;?©µÁ0\]2?°<Âz›-Ô?¦^¦—¬ì?¥ô©s¼?š¸Ä'$9ø3FGL J1241.9+0639@r'øÿûÎB@QZýç!À:{õ[aO¦À;ÈÎX%[?áTr^÷Å@^wڂ?üÄþÍ%?Ìqƒ£Á™F¿ê'äjÎ*?¬`Ÿ…ŸoO¿×åï!z=AGNbll?ïßó¡"¥?pâÖ9£Ž¤?/rÔ¥,¼?2‹îRÀ?nE?pk-ujÌó?ïʈ¥.u"?{«â,ivs?e/V@{–g?k{¼EV¿?p$H‡£Ð?sù¸Š;Ö?îìaz'2?‰¶7@l?†
TÌ?wÊCÃÞ}?—fˤ¡ó·?"yX5É?ïDžŒn.n?"FJA
'?SÚ,l'?b'z¯¤@?–.AWk|?'³'zç$~3FGL J1243.1+3627@`¡aՈ]@T Æà#Á¦À8i§e47?À:ùP°ò{³?ËQcøšÓ@@쉫æ?üM$þçüÿ¿Ý£!%G?ã¿×¹O»¿ØZé[!ܿӕ¾ùiRAGNbll?ïÚ6†Ù°#?pCçÈÞË?Ms"u›vv?J¯‰´C?nl°ˆèÿ•?n.Ž®'ˆ?¾=Ò?NÆ
«Æ?pœ¹Òè~j?wtÔtъ??€Is‡'˖?¤ÄÂÎ|?îUáwöú?™©+"O?Ž¨va•í?…U'ù±‰;?£+7Êè*Ú?•z«î3(å?íCoz=u?£Ü2#©Â?zP®á+þ'?€L¹î4À[?´BQ–Tq?£6îõý3FGL J1243.9-0217@r±µß덂@NDÿ΁ÙÀ:L}qDçÀ;Ð:FLëk¿Ç­Í‹Â&@t¿CLZ÷@|Ñ`…Pâ¿çùÄ­ù¿ÞÝD3[¿Ó½°"퐿ê"ìiSAGNbcu?ï®Ú\Q™‰?"5¼8Nj?}î*^?º†û?eIZ7º¾?j¿Y®—I?ï•7¤
=?ƒ·T}d@N?|­–$f[?|,
mŒ>ã?x¶—@Vz~?xfÔ¤N7?î<œ¬Æ<? ;/疇ä?£ZÜyºE§?™âq¿c»K?™³vò­9?‰ßíOòîÈ?ï?v.4öT?ŠÄBiÂÒ?q:¾†;[?pO%‹¯?"Ë뉿¦{?‡HDš€3FGL J1244.1+1615@r\:¿¹¾Ó@SÀW_ÍÅñÀ:6—ºœH¡À;Úe€…¿þ˜óï{xq@fÚ`´Ø@i1€«Œ
¿å±‹I¹vH¿äú–wâJõ¿ã*0¯dÿ¿ïÿÔ¸àÕAGNbll?ï'Ü:¶7È?²4ºÑ°"Ö?V'}±	Ç&?iéùÿˆã2?ˆÄœPÕG?²´šB9U?ï´,H%	?ŠyÒi{g£?h˜6¿·'q?s÷äpÚxp?yÀŸ¯?‡˜F®'oÌ?íþYÃaB?¢VÜÖBš?—ã€ôíµ?Ê½ Æç?¤(®:Ou!? BuÍ*îm?ïÁXÕ¼"?¥Útôã?I$>ý?]^¦…!¢ê?|3-
ap?€&¦Š^@3FGL J1244.3-4955@rÜ7À*ýÛ@)ÛҁA³ÿÀ:vãŒ+óÀ;ŠW™¿Ã?†Š•'@o"9櫛@{ÿªÅ'¿ê¥¸·Ó&¿¿æ[±9'ó¿àÃùòþB¿ÞIî±##AGNbcu?ïß&rây´?zª=õTÇ?;©¤jÕ*ü?9ý'"³ØJ?mdX+§k?yþÃc΋?îÒi¾f!ˆ?«ó–ümTa?sHÍjE1?yŒr¤"¼N? gzÿðžÊ?ªêOb†Ø?¼ðT?"ñUû'?†*s,Ïx?uòË'ƒ×?¡;#3Vå?'×ÇyâÁ!?îçMÿÑC?Jʈ£Û™?O ¡ªj-d?Pæ0Ö|Ÿõ?¡‡yC?cËÎö\3FGL J1244.8+5707@_. {5+@Mýþ +ïrÀ:PÃë|»=À<¸e6»~¿ØšËOkšz@(=}¥@½?fj¿å£éqè¿ß öÍ0 ¿è½)¼<ë¿¡X\|F'AGNbll?ï¡fAWÁ´?—CU(±?'Þ)'JÝ?–7°\ñ•¡?fjF¡ô?lé*Ùáó?ï¦õ‰š9î?ŽtPÝ?v•rôVàù?ƒ©f–ž—?uïÈ>Œ($?~Á§Ux@?Ð0"?'w±W'‹'?"h w?ß´?ŠBç|Õâ‹?˜G?†0ÌóÁ¬/?¥øb?‡ê¿çO>U?b.ÉMAñ?p÷¦—1F?‡Î$.—6³?†çÇۗÿ3FGL J1246.7-2547@rÙÈ¿Â"O@BˆÄ`Á
À6þBÍ*1À:Ï;+O9#?ûpF™ @"±M?@ŒL/Ùa†¿ànK¾´9¿ä"ö•Ú-š¿å˜©PŠ Ç¿é+=}[lÛAGNfsrq?ïÑïFÚ ?ziERñ³¹?e·Â¨^ïä?oÏæÄÆ.ï?hXö}˜îØ?q¹·þ5_»?ïÍú'ÈlÀ?yŸd÷óÿ?f@útV?lQ{3v*»?l—=²?qš—gˆ°=?íñX{"é?¡_ŒZùX-?¡j»rÐ?—Úé®8 ¢?žÿzg'â£?•¬Uo4D?ïÓ±JǚÒ?È‡EÞ!?:ÞªéŒ&?U¤¾¦î¶?tyoí™Ô#?'˜
 M3FGL J1247.0+4421@_fwž™@R0Ÿíp±À:šF…öN¦À<^â
¦²?í¯2½T@7—›è~@wå¿·æa¿æ9Öi>ï¿ë¨6ýHs?»(8¥°K¿Ó7âÿÐAAGNbll?ïûffyv?FИ^b:??%C¨nL?*lŽM?<ºø¿¨3?D"'­f,?ïÆ÷n-/"?_XÔI70?fΛªø~?s35Û±?qûa'ò?v˜æl¤Yó?ï»—'ÄU?"Š @ŠµZ?‰ó©Ð?ˆœ´øVãá?ï	Fjq?Š³ØŒ1Y½?ïҕ4lá·?|52Ò[ë?9ʖB¡©?RW†[>'?u¼hÊùÙ?zœŒŠ˜3FGL J1248.0+5130@_Ž`€sX@PgGÿÞrÀ:"HÊt,ùÀ<­»§¿êç
`™P|@ç	ç5@N¸@xÁ¿ëiĦ¿Ò|ҒÎ=)¿â&|§­¿ç©	¦ƒAGNbll?ïêúv{`?eò:w =w?_¨HÑòï?d…®&R?DÇmæn =?E)ùç[ÞT?ï»°Å=Lj?€Ý$ž5e ?mÀŸcg¢?rÀRìQHb?sGM¯'–÷?u]2Ÿ@ôÀ?ïøÔÞå?Œö""àð?Œßá|O‹¤?†	ñwLd?Œáé'8ºå?}:ÚÐܦq?ïÏŠ'NC?p='W|&ø?S
ìÞlá'?RÓÑò¸7?s²¿´½¦'?lÑ)ë#@é3FGL J1248.2+5820@^îÊâ°@McC hÀ´À7Òæ±z`ïÀ:ÿÕHœQ?â"èç#~ú@µO{é/"?ÿ(«Àb±%¿Ü1\~†Ý¿ßԒ;ßÝ©¿Ý…9ÿïÓ§¿Ü½œóì zAGNbll?ïÒ7dqÐ?tk»úëÈ?UÒ¬5™ù?UJ稶;h?qo¢äß±?q¬K¤\LÜ?ï
HIö?¡óRÍS7?'яÅa?—!§5£=?‹LX
÷¸8?"‹¡Ž¥Ï	?íÁâÑ]:?¡G%Hå¢#?'w/v{W?Ž¡'Ef?«&;4¼€Ý?œŒyŽô{?èu.?µKûE
,N?¥QžÌ¥ûÐ?¢IÕiMÍð?È7DDQ?´µþ†Œ3FGL J1249.7+3705@_6ÆÞvB|@Týß=À9³ªŠ'¥aÀ;m¤K¤CA?ñ-
¦®*@—üï)n?úx@HŸ¿ïÿÒ~p&?ïÿ#Ý"¿Çzß¿Û­KÄ	ëÍAGNbll?}CBF?£Ž¸JÛ/?vn@´Dj?wŸA> úJ?zCXª™?£$w¿DgÚ?îí6×ˊö?¤ ƐÆX@?‹Ìo2Xø?'ªió'™B?"råNõt§?¡º¼ýÄt±?ëã˜3Y?­CÔÃ	m?¯ˆÿÚ°"
? ¹ q6!?±#}æT8?¤_3ÞÉÆ\?ìJÕãP0²?µ@VRU×?¸9uìÇí?´UVO¡?•Á-¾FÊ)?œ{»T$¹3FGL J1250.5+0217@ræÀ]RÁ@PJ¹ßõž}À::¬¤8À;²I|JÔ:¿¿$b#ÐXŒ@Nò^@Ÿž¿ô!P¿äF+"Eӿ祐¾¤¿ÞmŸÌtÉg¿Û#Þb\§²AGNbll?ï'A±3Q? ÿ@pi?[5½`I?]P˜žŸ?›¾îö}À?Ÿ^㙭	È?ï¸Yå¿+?ƒñP¬:?qnÈ)ƒa?yBEï–P
?rΞ¶öç4?v
ÄE:¸?î'øÊ("?•OyRt(#?‰Üè¥í|,?y!¹¼a?¡Y94€¼?'y]bÕÎQ?ïE¾Ÿóä–?‰á•'€¯?]Œ
˜Ô›ë?_©²}g?•ok'ö#š?‰+G5©m3FGL J1251.0-0203@r뿀ß×@NhP`j£ãÀ9Ûs"u"*À;²7_ÞO?ÛdÚ¨¶ @&°™_^@ùf!È?í£Îxoê¿è±úŽ|¿æÆ÷ ¶¿æ¿Ê+€ÚAGNbcu?ïøZ×B»a?N hr±æ?6äCw´—?;½8¤,«H?C"bSV¥¾?HŸigžø ?ïÀiÚN?€¡Œ""í2?n›±b™?uˆîÌgº?p¯rˌÆ?s)Î,§J?îÎîy%—?Ô:TF?‹:"Âk$?€pKõ<&?˜ŸÏӗˆ?‹èµì›	?îçó'!'? œߩ?~>—q\J?xßaÄ*?›qùÊÿx«?žŽ´¼…43FGL J1251.3+1041@rî-?ž{@RcÒtwÀ:ä9ÐÜ&À;ÃSP	,Ï?ѧâõ$§!@ÿ™©ß¸@'‡?Ïε¿êiMk¿çõ'C‰¿×.FíØ¿¿áX•:íÅHAGNbll?ïýs-™?6OˆoŸ?•"-ùÌ?ך°Šài?1TŒûÈ?4­}´+	Œ?ïí/+î ?¿A»|.{?hg$Î8¤ø?u¢[h×^Í?qõÖìœÜ?wȨý¢^	?'ü?Ðêhӊ?pÇ1"/Ù?rt3'û8?"Z÷ìhð?wYΰWzH?ï²Çäxg¢?|ü«Çȏ?KD.¤ºÓ?Kßî"½v?™Ã÷šjC?|Iôt c3FGL J1253.2+5300@^"®ÀrKw@P9ßõž}À8U'ÙŒÀ:Û«8þNO?ôE!óé@µ¹	÷P?ûæÁšê|‹¿Ö×,>CÔã¿Þhvšò¾¿Þ}âw­¼¿ã8á…ÁuAGNbll?î±|ÄYBñ?¢K€Ö^?Œp÷ƒY?­M˜y?›—ëôJ`p?œ‡â9z?íÜO™?¹Šëblç?¯žøŽ|ß?´b îë¸?žÆ"ð±è?¤Ù³–º]?éó×Yܟ?°ë|9ΘÑ?³C¾šVk¸?¡"ì²ãD?½#jªÚ¯R?©*±[ͧÿ?á¡4ê1üE?¸ÏޙâÍ?Å)Þ;â™?·ïÐ'Š»x?Ò)	<~)?µ"e¯é8â3FGL J1253.7+0327@sп "`@P•€	¥›À9o™YعjÀ;^}Vlô¿ñdt
Ãâî@–«†ñÌ?ýwý%	O¿ÐV>Zø¿ß-‡Ç#¿ã,tè$Ë¿Àº½mU»@AGNbll?ïõƒr‡?S>ê¤??>"O¼f*õ?@NM~2¶?J±rYºÎU?M6@ŵ¿?ïÖ1Ôìd?u㯃ÊŒ?`'yºÑ?eñP ä™;?i?™á}ó?oՔƒm¨?îùYØž?a!ÖíX?2'hIæ?‡-éf_†Ò?';ÔñKgP?'Öò¶ÀW??ﶥ©Tˆ'?}¿žˆ?ðIGn"'?"öćÂ`?',µOã?}£ö÷Qjš3FGL J1254.1-2203@rüÀ?ö@Dg_ !¸À9¶ôöºÀ;"žý†¨ü?ÖXâíþÿ-@¬ã £Îý@]€k_ʿݔûùúÇ ¿æ1Æ=³â¿ä~ùlóà¿à^¬
+AGNbcu?œ5?¯ç23O?™ɳåw?­ y!45&?•¬'¸&"ÿ?—ò@f2?ïU©0[§­?'ç	ù¬¿?‡‰qxí0*?ŠšÏ¼·'?ƒBp(ä"?ƒ¦QZ­îæ?íé(¢nêá?šz}—´UÞ?˜‰-ÖÚéë?‰U{@:.Ø?¥(Þí£Ý	?'¡£»d¸k?ìïŒ\¡V+? "x\i"?'²´b·ºœ??¢z×ñ?³ÖðG_ú?ŸAOfÄ$_3FGL J1254.1+6240@^™"ÿ‰;@K9R¿ÀtÐÀ:†T‡@сÀ<€­9‰?ً€/ÿæÄ@o5w±…?þo'ßì\?ïÛýž?µf¿»w?"e쪿â܇hGDÁ¿Öº›¡ŽªAGNbll?ïØý%Ú<]?ƒx¶™•8Ç?pèD^æNx?'óìø{‡?DÉEŸÜÌ?LcájFÀ?d+²¾?›;ú'-‡?'ÍϟRoa?˜xo·¶GØ?x.«ÂÙ?|&ˆ}ÃT?îsö*ËÄ?˜ßwY.ø‡?žxT8ß8?•¶xAݙÄ?"æn‡W?€AI«¨?îU©×ÍBG?¤3øVZæ?ž*¯z"ь?›¤ŒÿÐd?— Œ4å{?šN²§Îân3FGL J1254.5+2210@sr>À¨@U?Ô ÄÿÀ9¹âÅ\–À;ªw"^?äxg¯*"B@
¹sólÉ­?ÿî_a9€Õ¿è	
£_I¿Äò}¼Õo¿Ý­HTúÑ¿âi°IsšAGNbll?îât`x.?¶Õ.Ñt?~é‰þœ¹C?Š,æ4K?œôIËò?¶?
yMâ?í¨€æ-µI?¶ópX1ô?¥NMq—Á¿?±·ûAK? )¤+Œé®?«˜…˜íË?îÞqYÊ·?›£CÎEÃv?"GÊÍt?…ôȗz ¹?¤¾"üš}?–οµ	?ê.«¥ós?²¹¨9>Ç?À]Lpƒ)?²zë¡g²I?« å#Þ¼0? §ßìø3FGL J1254.9-4423@rùŽ?þó'@2yMŸÆ…À:[®UéAÀ; þ"ÅõB?á¦Ä'6Т@
vêb^ïÐ@Žâà_{¼¿çlXç³ê¿êÀ긽¿ÓÓàò'¿ÄvÛ">ÝûAGNbll?ï¨ÄùÂ<?—™@òó¢?FTÎ͘?Qôd –?"i±¾71?ŒXeAhéñ?ï¡ódRŒ?Ÿýº[?m,%[+?p³·•*?€@[â%…?³ØÍèTÁ?î½[-¥,?'­«wÃò›?†s›s"U?x©4TeG?L`} µÙ?Äu0¤?îÄÕv±+?–ØüØ$R?ZÏùÍ1?m%%&c'Ê?¢Ü(ÕnƒÇ?–(FC±•3FGL J1256.1-0547@s†_•'Í@L‡Ã¤àõÀ6'_Tú-XÀ:}Uü‹×9?üãv$˜G@ ¯X	"µ@WæÄÊ׿â[#&9"¿æ.>¦Ñ2¿åHסßZ»¿ç:àH!#AGNFSRQ?ïàP4khà?lþ×ýà=‹?]Ю>û}¶?c7uzÄl?`Çtu`Î?c'T™š"ë?ïÛ2kz›Ž?u©Å·€Æä?^PRj˜,?eÌõDùô¹?e¥kP\ë?m~1¤‰?íI§o°?¤¸Z›Ÿ}S?œrVÿ³?–‡o…}?­,dÍ°…/?ŸË
áè+F?ï÷O›—õ?b™Å‰hp>úa1SÍ?/twܺK?PøoM³O?bx|a)÷·3FGL J1256.1-5919@røœ fè@VàºÛ^À92ÃWÙéÀ;Üæ"*¿É}Y†.-@5Í.œu—@X`d¿ËSiè½'¿éñX±¶µ£¿ßÀýFùIê¿áy³¤rAGNbcu?吮4'?Êæß×L(<?ÕìYk?;yÅþþH?Ô·¯TÑE?ÊÆ·"Ô¦?é¿ÕŶv?Ç\Ä kJ×?+wP‹¸?"è±:=Í?Æû:£Å°?Æ" ñµª?èSó"
àk?²Ëƒ7tÉö?«T‰¯O2þ?–*¿Ó•O8?ÇÛD±"?°b!Œ‰x·?éd4L€gë?©÷Qt?pJ´³=¼é?jÔ°rtÖ?ÉìÙ(drn?¨Ï-NƋ3FGL J1256.3-1146@s
…ߨq¤@I‰L߬£bÀ9—RMª­¾À;|ë Í¿Ÿñ|Êúç@Vô™špY?þƒ %"º¿ç³֎Ë¿Ô½Û Ø°¹¿â-ßÐúH¿ÄXPüXÅAGNbcu?ï÷íXJÞ?PÔ_Ì=YA?=-¾}ºF€?@Xõƒ	?A´§_÷b?F'FnW?ïÇՃ!P?€}bè¥R{?lû6 µã?zåZ5æYA?kfÁ¨K§?oY`"9 m?ï>)EÑÍö?†±BÇ«×?"¯£¹_?~·¨ÄÓø?‹ÆtÓ|^?~÷ƒ±9Ó?ï}ÜIL>?ƒ6•–íEq?JºãCü'?RÕßzo›?ôÚ¹m'9?'¬¥à]ö™3FGL J1256.7+5328@^I' ÿT	@OÒŸá²7À9Ñk÷Ÿß.À;'l	=–d?®÷û¸hSá@šZ]n›@ë@UZ¥¿ãì…g]‡¿êBÔíÇ]¿ä[D,L1¿ïÿåV9%CAGNbcu?ïìçš›í?xý¸¬ÍY?4z`›ü)?>ÍóðQë?`‰ÙÓ(?wü'–ª¶H?ï[^‡oÇ?'$ÉùPû?†ÚaÅ˜?‰
FáÜÑ°?'Mü†xöX?e†7øO?ïH½\äb?–©]Çj?Šç¾Ì`H"?/|N`7?'#î3O[?ˆÌl	'KM?í~9r–?¢¯›«¦y?D°<;¥?"²µÖ—Îk?¯¾zz¸Í?ð3Íbê3FGL J1256.9+3649@]×®6	@TUÀ%õ]À9 /ªèvÀ;Áڅ4?C%҄@¸'ô´@¡Ë`;)!¿Ývƒ¢êÙ±¿àÝN,çGU¿ãÇÔ©©Ì¿Ú"0žÙIˆAGNbll?ïô5â¿ã?rtЧRsý?=¸Åí"Å?Ii3'E?P3ÌN¾‹2?o¢ã('?ï ´½Ã‹L?&\Hÿ1?p×
ÝQ†?w±"êŸ2?~ΓA,¬?‰aªßaʾ?ïBç\ió?…ª‹"<ˆž?"ŽÎVˆÑ?}dó`²`g?‹=š,ŽúV?}:ãQ5Üô?ï_V8fÃ?‰ÌEÔ<3X?qÕÓ­·?pÞ$é›S??ˆY&óó?ˆ'æ¨"Œ3FGL J1258.0+6120@^`Ú¾'œ@K─U$öÀ:ÒÎX%[À<C"]È23¿êó"Q'²C@
Ì\Xp"@ÅQ *­¿ïŒ ÈÊ?Ö¥™§±_^¿Úøj
›ö|¿ÚKàZÀFAGNbll?ï¾kÊ­¡?"À	ƒ?}[¾Ð8?"‡pÅÃò1?KxÇXAÐ?Q~1_ž?ïÃÔF˜ˆ?}¥We,…?n8:r·?q"•3tÍ?nÂ~ôÀa?ržP_4›'?îßHxC?¤J2Y<ń?¨PAo}6"?¤Er ei?ŠG(<-¹?zöcßÂo?ïè^+Öô?d•5Ã-…?G‡}À@?F-­–õÔ?a¿õÌ?b"ó6¯–¯3FGL J1258.1+3233@[±þë-
@U[íöéÀ9‡"¹À;ÄnŠ!V'À¸gÏ2f@€2t†@»ÓÿÆõ¿åsôwek¿éÂÒ¼¿¨¿âšâ™èŸ¿åL?ôŒ¯AGNfsrq?ïîÊtô³?Y@¥@ÅJ?s?F?3óXjk'?`'ñ½‡?€ðz,…Õ?ïÍ8¸žiû?‡'+ÿ¯?]6 8Cd?ffö¶OB?r¢º:Í?†+}
±¨9?ï/àZÓ×<?°|ŽI–?ob]Ž{?eІ¢ŸžH?–¨óÂöu?O‰_ò?ïú½³û¦?P³%L Ì>Ó¯—»i/>í¯t¢&¾"?GѪ›\?Pœ Ä¡3FGL J1258.6-1800@sY_í¦a@FjÍØã\À8•ÜJRÀ;wU·Ây?挆`#M¯@
ÜæöC¿@'eÿ¹3=¿älŸædοæ¦(c©ü¿ä¾²¢v"c¿ê–ón¢AGNfsrq?ïì3Q¯?`-¶nšê?Y$X2¥š?X$˜¯U(x?LêÞw‰?K˜€ÔÐ?ïÇ¢õ¶G?}]ß4°£?k÷n<´?q'5'±ÜQ?lòN÷Û|p?s*fxÕ¿?ïF¡åç2B?'2a@W,Œ?Œ,ªF¸?r76|wÃI?ŒËYÛì·V?{‡jAý?醙^Æ?';ÇÖuR?UfpîÔ
?VÛ ìŽ+?'r<pŠt?•>z©[3FGL J1258.7-2219@s£¿ø¨ô@DAMå"mÀ8®ºŸ¹À;9&º~ìo?íËùÁS-@Ÿ=⎪þ@¶?Ÿ¨&z¿ã¼²ÕÍø¿äº1"X¿çuJ%NT]¿åB!´ÊfZAGNfsrq?ïÙ~îºú??•½ÛЎ?a
è¯/ò?dŽ¬ÐÎ?es(•Ö¨‹?•£áO"]ß?ï­hUX>?€Æ"k"úU?tàm.æÞR?t€Álr"?tkh$ú¢?uš«K$±,?ïáQõŠ?‰Ë09Õ?…ó‹@š?|},PûP?'ÞT@.d?Ä31ôç?îMìih
ð?>Ëöà?†Þ/'L?'J¼YR	?¥ŸÁݺx?›¤*BÿôÅ3FGL J1258.7+5137@^¬Óª7@P]‡ qäÀ:±äþú2À<Й
'¡¿þz5
(¯@
¯¼{F@E$¿ÒéG¿¾²lƟ-¥¿æ1±3ÐMF¿æPöñ5Õ¿Æuyv/ÿoAGNbcu?ï¬åhÂá×?›¢ž­2;d?{‰z;Ú§)?š£ë¨Ì?l¢ÅhÙ¢?tsiÌ/Ÿ?ï×Hóàθ?wœ¦FûiI?a`­OÄ?k>jR[¢i?g«røK?njÑ\$Ç?îN?™ýù¤ˆ¥? Œm*>g]?"Õ‡š·?$Ûç oM?ˆGhš†?ïí/ãòƒ'?cvŸ"*Ù>û-´æeä?Ô0'®Å?b™Áî{?ceÙ¼Å3FGL J1259.0-2310@swß (@CÓÒòäÀ9·ŸŒ¨À;€Kµàø?äôÑp@§ԖoÄ@:‰à>¿¿Ö€ºÈñÔw¿èS$Ê\&"¿µük­Ålþ¿ãM—"þ÷AGNbcu?ïfDß÷Ç©?—º¡ù,Ïú?pz~×xµ?sÇ|œ#OE?Ž1ˆ–R
w?•ÑÉÑg.?ï8‰ ?[È?"{¹:²V´?g¡½$õ?äšóIM?"Ü0NkèÏ?"q†v$£Î?î¨ÈNª¥C?'Ytò"l?ŒñI·¾º?¸\µ"ßO?œnQNËú¡?‰cMƒ._v?ìÑgùÕð;?¦Ž‰|"í7?'}3W'ä½?…ÚA¡Šá?·%Æ^AŠ?¥tm¤|Ŕ3FGL J1259.8-3749@s/hی@9$;I'À9¢Ö(–!?À;ŸÛÔ§Œ¡?ÙfJ`»@où¡A-È@îø 7­ì¿ê	‰…i%¿ßÔ«±|ÂÒ¿á&ŒÓ|X/¿Ý†ª,þ'AGNbcu?וּ	•¨?…~
ҍÀ?pÐg@²›?ršr#Ø?xÕ:ƒg?€0G,]¸4?ï81ÌW(?–ˆ^©dUç?Š$ä¨`?Œ[Žƒª?‡Ï§hèm?Œ2—ĉˆW?îE(,óë?™ôúvd¢Ñ?–'8ÿW?‰•NéþÛ?£úý¤¾?"{9»ê?팳æ€&b?
 ŵ.?äïhCÙà?Œý¬šÊ?®ÂIãÛ¬ä?™"%ø‰ª3FGL J1300.2+1416@s‡‹À]RÁ@S?ßеÀ9L#Ü~¸À;®d¾£?ÞXìd[Ž
@Œ+·ü1@×:€.Ž‰¿ê+°#"5¿ê©ó~'W0¿äïÉíÛvo¿ïùé÷¢AGNfsrq?ï÷Vd§xM?sB²´J?3Ã໋ðÆ?3'Ü5?HÄ}XÔ²?s.À‹‰­g?îëNoç?¨¦<™²‡?—€´&i"¨?$ÙèSœŽ?–Áâ¶O…?¢ÕŽÏúˆ?îäöZN"4?'þ]ñ$º?Ñˆi²Î?†uspyr'?'¬L‰+Ï?®/X@"?ì7«%õ9_?¯JµCË5Ô?²÷hJ­­¥?©?¥¥UC?¦–}Q×? ˜_}­ä3FGL J1301.6+0832@smD@lÚ@QÐGßþùÀ9D`Þg)À;¨âøˆ<z?î…У_ÚË@
ÙRl3"è@@dÊ¿àWe¿äºH«ÿ4¿æE3w•|˜¿ïÿïʆT PSRPSR?ݸԇºó?ÏtSýK?Ôïáօ`q?È+ֆ0Ґ?Ê®"DµÉ4?É$ªÅöª?ÑK">mˆš?њ^zJ?äÀ!j¢;?ÒãïM¿c?ºµuúôËÃ?Á~ ñD?ä…\'Ç?²¶ÝÒ~@ã?Éê+n1ì?®7Ù0¹S8?ÄÓ
ò²?¦÷IÍ9ñ?¾ê«[?²ià·ë¶'?ê/m]JK?»wžÁy¡~?¯3OØüž?ªgMOÍÒ3FGL J1302.3-3259@s;?¦Þü@=ÓÝÿú÷ƒÀ94¹šûÀ;'h§‰Fe?ý7ùÁw"@
vêªÙ2?÷…«'	?ïúŠˆÏr¿×Ð.½§¿âwõq©¿í`ö0ã PSRPSR?gu•¾ÍËÝ?l^q°Ã 2?ïN¤:')?¢Ëk˜=ˆ?"<ÆTU?¢6&k"Û?y€>ì^‡?‹œØ£p®?ï©6LR}?¦P8Óä±?—ªÉ{^?£Oð?k e?§½…<\‡+?™2*âqù(?ëRL¿Í¤?¨F+ÛCÉ?¹Ž×ciWU?¥3n#?•ptGüýç?}&r!'?îö\ßE?¤–¯ÒZM?¤è`³Œ¼?ŸGj´Ëg3FGL J1302.6+5748@]ÿò¾ÎÝH@M \ßÔçNÀ:…6ÍòfºÀ<$y'¼U†¿ª±›aþtP@;*Å{u@-_§°^¿ê¡:fпæÍ»
hÊÖ¿ÓØb<`-'¿Üº¯6*èAGNbcu?ïø·º*'?Uæ0Ù‹ª?BÎfÄd£ë?T=½Í°Î?4ª¤¥åv*?4™´?*†?ïÁ"…ð"?Þٗ_"?oˆ}dÿØ´?y&Xþ—â?nä}'y?r fžzÝ×?ï-­	ž\´?Q¦ºÓU[?‰bì4^¬º?‹öŒ¦'ê?‹1Ñd
&1?zÔó,!õ#?ïÏÊÎê?t~¡O¼•P?:Ó<zç"*?@ìn>¶DÄ?vmdÃÿ]?sû^'âi3FGL J1303.0-6312e@sÃ{á"¿Öâ:""•À8'£¥AÀ:NU\Rç.¿Ù™bìc@Æ_Ȓ€v?úDå)?ïú-Ç©­¿åhlÐ㳿â1¢4rÎ?Á!™h§^OTHERPWN?·öéìqF?½¿VâÜ$«?{ycÖZ©Ô?aä|
?ìÊ0u¼ƒ?¾ŸL5ü{Ê?Æ'®I8™?Ðx®h'g?'×!ÆŠ?C—¼â~?éé¾_V?Ðlü.Tö'?Îÿ?©‡bS?±üø»zp­?³RR×b«?žuØfÃö?åÕí«C;?³ºH­¿ì†?æy¶näé ?ÄoȆ!'?>2Wlï^Ù?LFK°b;Y?ÓŒZñè?Änñ]âÛ3FGL J1303.0+2435@uՍ@$³>@U—‹àôÀ8‰ñ…é¹À;m˜«]|?ëÒb?‡¡Â@»V†''@r±¿€3¿ØÁ'H¹Ï'¿âú¦ôÃXQ¿ãڔßÜ°+¿äNÆýTÿâAGNbll?ïôuð™3?^ÃäŽF܀?G2&
"	«?Wã—ƒÉ?HŒ0*K?I¢© òÞÝ?ïÎgtÝù5?'Î_nG?a#¯ÎYm?oUñüœÚJ?p:mª8ý?Nø|ã‰?î馡äŸ?¡ðÉx?™¬vBqp?…ÍèÿDG?'þiP¢3p?ƒòõ0Õ=?ïéÆ!"Å€?háß±ñ3?2OØ·Fºù?AäOz]®?cïãdQ©?hrJ"3FGL J1303.7-4619@s~KZ@0ñ'lÀ9t.¦¸§À;ŒËÔHµ¿çƒÑ¡¦a@+‡ø[Ç@]à
Ü¿çhc'\ʗ¿ãÁöçÊÌd¿çfå\š=¿ç@>"iPAGNfsrq?ïÖqX9­?|aŸ—$;?e^mck>?iD€¦eF?dƒIXï-?u5ub¢Ÿ?ï¦9»³hü?ˆÊ[V˜?gvÊ~šwÔ?i7aïQ€?€"Þs"Ú?†';æTF?ï <8B¢?ˆooøh?ºÈˆÉZ±?sÏ®0XØe?"^"4'þ‹?ƒlVx¬e?ï:†œ†Ú?‹Ñ' áÊ?T2xŽ(ŒC?UD¼þÃHv?—læB6®?‹>&Ø[È3FGL J1304.2-2411@s*³ S\ž@CJà€øÀ9¤0íCÀ;yIoH?ê¸-ô¸Å@¶ì²Eb
?ÿPò@¤µ×?ÕPHÌfdR¿ØIµ‹g§¯¿âAÇÝÇp¿ÚØ/ßõ&;AGNbcu?ïµÿŸ'g?¨éÆYœ?wÝ>tºš?vª4…ýA?jF_ð¯…é?láÁfH?ïuך!]¤?Œ'ÑT ðy?'ÑFÛ¦'?ƒÉ¿I°¶?ra™à"?†í]?â?îwèñš&?–&—$å»?šçí&ïÿ?¿làÎ?–7µºÜ»ä?"øù9ñÝX?ìgne)?¨ZcE?¢g³ˆ|X?œê'^YE?³"X5H˜Œ?¤<±èBõ3FGL J1304.3-5535@s^¿¨÷Û@ö© JMVÀ9xþï^ÈÀ;-QîÊN?õC5Ú£@'Øì?Ùµ@'/ÀbY¿ßðë(ò+¿ì¤¯ÿ;_¿çJÒ6C3¿ÝßQ‹Û7kAGNbcu?èi#ëcû?Å
.®´?"I`—I$?½ ¨Óxa?º–$vMá?½$óe%Ní?èÌXkY µ?Êþ'L.(?ª—"Sl‰p?³—)Nþü?Æ(½=ÀZÔ?ÅÕ^Þñ4.?ääÕõ×Ñò?²'Œ{@?Âý=ÔÓöü?¦_¦­™N?ÉojSÌÁ:?­òuå?áï|m=É?ÀTØ–ðý?À'éµïØ?¿6ª§=d?ÓגJ	ú?¾XþÜ¿3FGL J1304.3-4353@s[ߏG0@2逾À8D7guZÀ:Úá& %9?ä³i0Ü@D‹çTbƒ?þ…ÜiM¿àlõÈÞE¿Ù1Ídn¶ä¿ØÕN\j C¿à'Í2|AGNbll?ïïÀ½ô*?`±ô¹0Ð?4à­n×ä?7+ñ½'¿?[FXÓ¯ù1?^þ̑nE˜?ïš}ù¹?…W××8?s–3ÁLÍk?r¾Aúß?`B)W[?,-h¬ãÅ?îóLX0d?"»K<½?½0Wœ?€4 ö°·Û?˜·ÜÎ.¦æ?U†¼ÈîŠ?ìC®V/<?££'/ežÞ?wP ³WâO?tÀøŒh8?¼mƒCP¡?£`[ÝÛî3FGL J1304.8-0338@sWÿŽÀù@M†ÿ ^¯¹À:ažõ!À;ʆ`ñ˜¿Ì$Ǟ±ÿ@1mÇXÅ@>€ vÿéìÝîœe¿Û©VÉmû9¿çñÊ8%"ì¿ÊÔ¾!¨
AGNfsrq?ïù¹³­fÚ?JX9ªÌÔ¾?Ce>¸ïÖµ?H¦ºË	È?&ÏÊEÓ?#'Ïõ?ïÑBµ¨ñ?zÉTרî?e¼ÇEºöÖ?pù¼Þùë›?iƒ¹œ.?ngë肔l?ïMÈ,>¶|?Šý€ßøŠ?‰ºÒºé?‡ +ë‡d ?'Ó"5Áw²?t›D–¾?ïäâÙRR?f㞂ðùÜ?+®»N?4ü±o:[?j9Ò:üÌo?fjÚLçCÝ3FGL J1304.9-2109@s2"@lÚ@DÍ0úŒ#À:7Ϗõ«éÀ;™S ' ?ќ®Ñ(@¥í¤ܘ@.ÜÿÊÐô?ïÚbð÷4¼¿ê.f›Ñ"l¿×¼<a/Dç¿æ2rgâ¤AGNbcu?ïÄý£ü¾?œúØKû°w?@xUÕãzŸ?B3k˜?{rnóE1‰?œòF­âñ?Q¤¨ú?£[k<ƒæ?œRM1½Å?žˆOLC[?zQ3[° ?(fijDù?îfôUF>?'öI¦?n×£¾ÊÜ?~QT,>Îî?¢5!»él?,¡ˆZ?èfS°k˜û?¸†û[–zÍ?§³ìXŽf‹? ß)!ئ?Èy¶(.q?·˜/,œ¾3FGL J1305.4-4926@srÿÑÜ×@*¿?>Ú0cÀ9 ×{|xÀ;jmH÷Q¿âU©´]®÷@)ê'/—ó@j`_'5¿å²À²W¿çXÞ=¿âÆì]¶¿o¿ãõç]qËOTHERsbg?ïÈ
,–‹¶?}T"Ö€a?e©%3ù?hÐ}â¯4?q&Vì (y?t.pPäx?:eæc?ð«gl®?sÞq*–'?uñ4,=â1?ƒ¥øÑ;aË?Œ&ÝÀ¿Ò¤?îOh_Æ05?™Y‹ÁyÜ?'¹°°y^?…''Íځ?¢,¡«•¿ï?"h®±ØgÐ?î3"–X6L?›/QÛp?e4:D7žk?cÚC¼?«srö9!Q?šu
ç‡Í>3FGL J1305.5+7854@^"‡aˆ±@Cæ@;YrÀ:	!0Ò/ãÀ<¥šXÜ:¿ï¶ö˜'ö|@
Û'òã6ò@ߚ¯Ä¿à¤kTôÏ¿å€ÚUÌ¿æ+ö8+¬¿ã™{!ð{åAGNbll?í[Õ(LŽn?º×"m-T£?«~(°á£?¶Œêsò"?‰	–Lo?¨Ò®šð³h?ïF†IŌ—?¢Ø✰ñ?ˆà©ˆ?œaÌ°ÿÆ|?†\O®™0·?'H2K¶?íZ€'}v? ˆßý0?¢ë–VI?™ ¤>Œƒ?§l`hÒU¼?"æÈ¡b_?ïL±'€?øŽs̞?jc(ÖP!?m÷FŒ4?"&aW55¾?OD'D9…3FGL J1305.7-6241@s	&ÿ}ú?ÁúŠ ,…ÅÀ80·omv%À:E\jd!é?㳐Núu@r¤@;¯@΂ÿú Ã?ïüÙ9™m¿âó^œm‰p¿ßÊ'Áe¤¿æÃx;%OTHERsnr?Á ££—Ƥ?¾€Â©°xÆ? è_¬=oF?¢|×Ê!˜¸?ê‰QV7b?ÁAÂ;B<?¥UãeàY?»~¥WT{a?¨ŸŽô
?¯¿"‡€1?í ©µJaº?Àš¢P? z?ƛEiY?¯\ÑL¤Þ~?»/â4l?¦ññ›ê»õ?æó^Íã_?²|""È>)?Ð0Ïfwí?¼àU	níÓ?¡2E/RsÓ?šCÿr
q?æÔÍEWœÌ?¾èð0çD:3FGL J1306.8-2146@s:É?¯Bx@Dyá`xÀ:I9¸ˆr*À;•"ô έ?Ô¸>Ã5@¨ÇÄû@@,Qy‡Ö¿æùx`}²ø¿Ü÷q¾*À¿á¿°ÁË´@¿åÌÔ^çl
AGNbcu?ïË9ÿ¨Á?€V]@ɀ?dÇ·MŽ9?j€3ÝtC?p<Oø­¯?xïÉŽ¡?ï
¨«Rät?˜>fÀy¹?'³Þ€2Ä1?'ˆ¯'ÂN?‰.*áZ¡?‡ÖŸ·oÒ?î­iãß?€«ªâ< ?"°¼Ð`9?Rߥ7{?šÁ…%'Óþ?‡Í4ô²?ì5Xdå?¦ð96S¨?¢ms¡wË?–~åÖ³¼?µƒH
÷?¢ðŒÑ	)x3FGL J1307.6-4300@s!] l‡@3Ň?úÁÓÀ8yÜ>Y×ãÀ:øž0Ø ¿Ö3ãVüæñ@A×*É­3?ýf	AGH¿ÄNñTÁx¿áæF!'9¿Óôõ~"¿×´]a§\AGNbcu?ïËZ"C¢?€"­Lã°S?Iñ¤3ì/?PO›ŽC)?w>žh`­Y?}ú¢D:?ï·ÍðoÌ£?ƒÚùiQÙ?i"»
û•±?i<³‹pÞ?wO*B›ã³?€æ"–LD?ííZàˆb?ŸK>3ž
?Žhŧþß³?")ª ÙYn?© "wÂ?›Ùº£'~?ììz\r? ¿‰yäÝ?LgÙþ
P?TçdLU…?¸c*Oç˜X?ŸæÜ9ê-3FGL J1308.1-6707@sþÀ//˜À4›ÀzÀ8kË^7üÀ;ȯ0ړ¿çÒ:"T'@"ÿŸ‡ð@™ÿ…Vl¿ä…H=JR"¿ç_ωÿ¿æf  Øxä¿år›ÞàæAGNbcu?ïÓ¨Àîoù?w—»Õ_?RþÉV\Ä?QˆLo,ß?qªßÖrm0?v
¹W*¸?î¶eWËy§?¬Ñ'9èé?p*•üùKÝ?iÑUçA?¢"Wé<?ªU€­­½O?í·zh¶fT?›‰˜0ºdã?"5Mϯ3?†MŸ ñêR?ªmØM±Ã6?–$—Ü¡?ï,-Á0?';›<qõ?.y¨äb?=]ËaÞ*?š=TÁ4?'%%VKε3FGL J1308.7+3545@Y8¬À½ÊÑ@T'Zà f¨À9®"ƒ‡ß]À;߅¨K
E?×ôNšÜ~Š@zŠô[é@ÚD€"
¿âŸ ®1'¿ä°ýëü¿äNdíÈùa¿ì´@d|´åAGNfsrq?ïÔ¼˜‡‡Q?Œ:&–Tá?bøÎH}Ð?fzSR8€Ú?hJ™Z01F?‹aúHF¨f?ï¹Öï?;ª–Ë?e`X×¥c)?mÙmØ ø?xdҜeE?‹ü)
÷‡?îM¯RTóm?›Œlþ>qa?—é¸8 ?0l4ۀ?ž`]µaY¤?•êÂvýܛ?ï×xEØdr?s·Í•»uÊ?SÞÆ
ãh?Yàqø"tí?n˜W–@?q®ïÂېË3FGL J1309.3+4304@[Έ~¿"À@Ri*ùš‹À8¤D¡À›À;Cä1m`V¿÷¥Ýað_ú@±«3J?þù_Js¿äBûxdsP¿Ù|ÙW¿׾íñµn¿ä ËR+úbAGNbll?ïØᗨhp?ypG'NÞ5?UPV°l
4?YRXi'A¥?lv<ÿaˆÀ?u2Ôòf?ïª9G*R?ˆYÝ.¿$Ò?qj&ú':À?zÛ!—~RÜ?yyVáٛ7?dø8ßD?îs,T*°?–$Ê;2$?_–˜L+?ƒÍÒ²½—? õUKŽ?'ô´‡ã?îô¨;Œœó?˜ëÿ–ÖQ ?S…WÌ,@Y?pÛÅH9%? QˆÔÎÅ?—Å	y‡õØ3FGL J1309.5+1154@söÍÀÓg@RŒ "µ7À9¿þÆDÀ;®ÛÇ4Ý?ߌð;Å[@¶EF0@%6€o§?î2†wÓÌ¿äp®·h•¿Ô
Û«X*¿ë®Ž
ÒÚAGNbll?íïyÛìè?©>PÎÒfø?¡ßDÙvü?9'¿èÛY?žR<H°&?¡»­€¨yÿ?ë¶Òmæ?ÅSÑ(FLb?¸ÐrŒªZ#?­Š)æXò?¢ñôâÑ?«ÿÞN8_Ó?éç-ã¬H¯?®´÷ íÈY?»ËɊÜ+?¤‹^n¦jA?´úÇWÁŸa?¤'ËWe\?è‡gËâÉl?¼Yá1Ë@?À¶'¹KôÚ?¶•l© P?ºXr.QÊç?²Î*CŸ‡3FGL J1310.2-1159@sc@@IOjNÚYÀ:4Þ]	À;§£3vO?Á"Ç<6‰v@
Ãvõ׈?üÂÀ¿xPt¿èãeJ\š‹¿Ð|û3ßοæÒYÏ:w?Ѥ\&'²AGNbll?ïµêcÎE?'_äð2æ§?lZ™'ªüã?oÖџQ¢z?vÝ¥:C^Õ?{e
¥'¦Õ?tL†?‡J`2‹‹á?rA'Ê},?'¤P¢ª?mé¬Z°?rÞÿðhq?îÖv¨¤?ŽáÐïÑG–?mGÖxæ	?ƒÅ`=Œ?"Ã÷Gk?ƒQ¥"·R€?ï—å¶f N?ƒüŠøʒó?Vb£Š.Ñ?dw‡·¨e?‡:N²¦¨?ƒœ÷JÅp‹3FGL J1310.6+2446@­öàF§.@UFãåîÀ:¯3‡	WÀ;à_?³UX²Â·*@
U¡¶ž@jÿ¨AR¿è´ Â>¿é)"R#J¿Ý)nÛ¢J¿é¸ÞصZ¸AGNbcu?ëÅ4Ë*f?Éƙ-¤´Ÿ?qEôΨÇ?|š&4›>?À`ý->q?ɈB³èø?ï+‡"ut?¡_!†ï?"iÛC¹Â?‹ Õ´'?Z!ê¯te?ªdÑLîö?í,Ý7ÈA?¥:mÿby§?•{Lj-á?Šñî©Ñ¤T?±@ýû¶E…?£1ÇN…œ?î§#ó'Ü?—·ãž|©)?‰³¶"ƒ?…$T‹Ø?ž—'²Îƒ?"ÈîñÝñ3FGL J1310.6+3222@Ugáßîè@TÓ¤à¹)À8éqHA¸À;2ªýo?ô6°x®<"@IG¨¶)@8ž_&+8¿âr<Í)®¿ã`=þúW±¿äjg="¿èºùŽ‡ÿAGNfsrq?ï㩌ՐÔ?dþzÒŅa?^<÷‡zÏ?_ªä-U£¢?ZoîÍÛܵ?Wq>ï&"6?ïɺK5?†‰ލ®?`'M# ?g<j¬ßú»?sÖ'êÏ?…IÂ7‹h{?î¹k¸ü½í?"¥ž9Ò?""1ªu?‹Än'`n?"ÎôÒ6˜$?ˆKʵœ—ª?ïÚXùCÙ?uTÝ2DÔ?GB"ªtpš?^á¡?oÖe']
Ÿ?sÁI"X¼3FGL J1310.7+5515@]I^_0çÿ@NÓ# 8ÜÀ:V÷~0ˆÀ<
 Òrÿ¿ó&—ºo@¿ênô)ˆ@7»Ñ+¬¿èi>Tpè¿é¯"4LZC¿åjY­"¿ÖÅZ¡¥ñ[AGNfsrq?ïý)uF-?HDë&¹îb?%µ•·Ø\?=É#Ä®"?'³åWGË?68xÚNhò?ïÙcigì§?uºÍÈ?b$òpù?iB™Ül°÷?d—q¦è@?h±'Bi•«?ïx£ƒ¦?'½Í¾òo?€#Fsá}%?€üá'ãwT?ÙЫ>P?q1ù¶c/‡?ïöÂáRº?RÍÆwaߛ>êÊâÁcý>óGËQY+?RD§–b~?R¹Nzo­3FGL J1311.0+0036@sB¡ Ï@Oˆ×ÀEÕÍÀ:¦.fDØwÀ;­À8iÓÙ?›j)?@vwY}Ë?ø¹€C‡>?î7¡Zî¿Ð
µ|Æq‹¿îw}»þ¯"?í0ÿ1#
¡AGNbll?î«W¡Þ¤ª?§†°Ÿ7í?¢Jòó6í?¥Å8§~åL?wüžqóš?†Šhži¹?ï…àõRû?†sFøþ!»?pP)C܌?[æNW…?lÙÌÔ%Lñ?rû¬*LU?êáÌbfï"?ª1CTc±?ºO4£oÚ?¦#?Û0Š,?­DГh'?™Ifw8
?îTJ°í½³?´†8»€?˜î¦½-i…?°³!|(?œˆ%à?§@Ñ÷P©­3FGL J1311.8-3430@s;0À&Ì@<.Bßx üÀ7vßY—KÀ:þ™‰©aŽ@ŸêŸñw|@ª1ëàcX@Yèb|¿ß\-WÑù¿â`ЛŸ"l¿æ!±U¢ô·¿ì?@]EÞåPSRPSR?ÝÍñoå?":gý{_ª?ï¢f§[Œ?‹AkoŸ¾ž?mݾŠ'×?yc%âgX?}5^}ò',?"E‡'ƒÝ?ï3m)h?¢Èv߶?"ì:»VI³?˜­7:B?Àô–% 	O?¨Õ6uυ±?é#ÿ¤X±?¯w"åó;?´ö֑ÿ¯Ö?¡Ç+ïAà?|?ØQk¾~?víºW¯?î©JÑý'? `£´ÁØe?¡ãdزµ±?yŸ–ÖR‡3FGL J1312.5-2155@sVŸ¶M@DV}€^_1À8¢kË*5^À;9ÜO σ?ñlP5L"@Ž©-
z,@™#@¡Û²¿Ý©á§òš3¿ÝŸ^Ï('¿á¯ýã¿ç:ˆ»ê–%AGNbll?íïR‹Õ?²4§"k'?¢5÷©€è?¡Û(Ö ?©ÏM;ƒ¢?­*Ý:J;0?ëW ç.¶?·¼È¸-†"?¾hºzåÓ?¶'RÃîÊ?¢¼|—I? ­Ð­v?ì< 
·úü?©jô;ÏÂ?­vù)7?ŸïÌû?®ÇûI4 ?ž›38wÚî?ã±ã…¹ï™?°´õ¬g%0?Ë$õ¥>¿?°Ì÷±ô›ž?Æ|D
Û?®*©C3FGL J1312.7+4828@\We^(ªC@QiÿãzŽÀ7Ägˆ¥UÀ;ýG¾Ûs?ð¾Eہpƒ@ lf*"Š@Y?ñ½ß¿Þ.3>ƺ9¿ãØ:Ö.#¿áNÊwvÈο䝞ö>¤ðAGNagn?ïù۝椞?BZV"'è?(Fy QþW?#•õý•·?BêY…?@Z«ŒS?ïÚŠ*	þ?w÷ãûþó`?]Šó-qÝ?eå
 g?gr0\_I?r®Þ"Š‰?ï9zg ¯ì?Š!þó?ñ?€û,ºŒT?|¤.äc²Í?È5…Œ¼`?…93ˆ|?ïÿc™ŒÖ>?%ÿ]SÈ>€cGQÑ{>šŽoæPÓ?"œÁª
´?%hÁY¦•3FGL J1312.7+0051@s­›6†¥@Ožm?ž{À8Óî{s=åÀ;‰Oçžà*?ÿˆ¦½@°z‰^
'@öp
Y.ð¿Þ¤ÍÔJð¿Úï}XgÂ~¿ç¢o-Ô¿í9"Paí0PSRPSR?bæ4ëñ;?^˜ß؁?ïÍq˜ÁN•?yDšûÁQ?o¨T	Åx­?t¸ÖUšx^?¦é•Ÿ‰+å?»QÕjk"?ìé]rjÍ­?ÂúÒÆf°?ª€"9ÉùO?¶Ñœj^?¸+'nýÅÂ?¥ÕöOA[Â?ë$Qo¤÷-?§áÌÛ †ü?­cä'µ·?"ôò¯•&K?H.á갟?ƒÀqnxâ…?ïô¦Ák?""ÖóMë?«ezCÎ?‹N/<.öA3FGL J1312.7-2349@sS6@c^@Cdó=<¡À9£úoFÍÀ;gXv¹šÁ¿î6÷'`¹v@tÎ0?üÒX_g™—¿éS''Õ¿à"ú Å‡ß¿à1oóœ´?²¯'ÓÉ/AGNbcu?ïôJ¤0?UhENÖD?6þjœ_Ï?4)ÙíE‹?Q¬H¿­æ?S‹ ÕÀŠ?ïÑjØ\øN?xðOÿã?c+os´V?iÃR^p~?ki¸/iþø?rjKó]à?ïSA¥»?ƒ§©}Ÿn?}ñk§M?t8eÈκ?Œ&ùÐÌ?{¨iù?ïИ'©Ê+?qVMN>óS¹ð?*²×ú¶?w c/â?qmî0MK3FGL J1312.8-0424@s'#ÿï9@Mé_ªŠƒÀ8ü2Q‹ãÎÀ;"ˆTÍ·®?ßý»Õ"Ù@Ø´ž­ªž@åÏ_¤*l¿âvÂé—U¿çRhÉþÅ¿ç Q¾+¿äâ!…U<AGNfsrq?ïøþ¸ÉÁ?Ne*'tC9?1Jtž–™§?Aô|iH¨­?Cbz͍¶{?D¾¿:¾áŒ?ïÖ,:&'æ?xw'gtº?d(p"]?mç	""0?e«U·š|?l"ÎÞ²j?ïUŒ¿h ??ƒc€¬ðÌc?wQçdøÙ?k)ЄŒÝ?ŽóÜs{ƒ…?€(GGmg?ïôV'ŒR~?`SüvlVØ?
FnoÁ?Õ¿š*·?V~à³ç"Û?`óÝÇE3FGL J1314.7-4237@s7üÀz®ó@4	›€#¦ÎÀ:Edè·äÞÀ;Ø
°÷?Î=ÊïZžæ@u!àO‹"@¨_–¾s¿çš»…Û)e¿Ý‰áT2 (¿êß¹Yí¿ÙaÆ¡´AGNbcu?ï·­3áÙ?‰T›í'ð?|Õ|­Ø€?‡
o5™ke?`²§ÒÂtŸ?gXŒ["ÅÁ?藺m«TK?†{$
7·‡?qÉ\3Â4?vZdpÜÕ?z^«Î",?Ñ4¥€?î±è,P?"»{·$˜?•Jyç`¥»?E\¤Ô(j?"x€Žœ¸!?'J Þ?î`ç¯C_?qzQVÆÒ?'33‹¯*?½^'C\Ú?¦ž¨T"?›sYnt3FGL J1314.8+2349@½Ðÿ·ZË@Tñ9èîlÀ8ß½×fƒÃÀ;ltK+w}?å±n Ø¹P@à÷Gʙí@b,?¤Ø¿Ññ¨Ys¿ß¥!¢'¹¿áÕЪä¿á§ÊlÓÆoAGNbll?Ÿ:è'?…iŠò1|?|ig0&=é?xÉ'¼í•?y·I2e®k?z)3Ò?î^w|È?°ÿ¼R­?šB7{¶?¢¾V\?™û–ú
ë>?§Õßlã¥?í³‰?úb?œ*pVûê˜?Ÿ³ãÓ*K? ô/Ýc?¥Mzļ?"øÄR»0?é.nÍÛ?³¶Geã?¾¶¿Éäy?²¾·ð!ß!?¸oП¿¬­?ª‡%¥ëh3FGL J1315.1-5329@s(`ÐÕ@"p'`@3À8Π°P%À;7€ KÏâ?ú¤Q›©@C¼«Âf@}KCuJ°¿áS-ë[êH¿æî¸É÷¹¿ê£Ó€‰ìí¿ïþ[2*ʄAGNbcu?ï$ž!ˆ¬?œÙ-»Lž?†4Ò!Ò$?'ÇšG÷?b£2¾\?'Ñ̤ô\?ìŸ'_'â?¾š4€Ï¢?¡3)"æcf?¤
rËó Q?·YqûF?¸PËR­1?ꨪ¾šw^?«‹•Í^`?º7ýM3OW?¤÷Í	'¾?°'¬½øõ¹? ¥ŸHPçþ?égµZž²?´';ù¿íÁ?¼s ÅòÉË?²kcˆ±é§?»)¡8@¢?¯Àé±bE3FGL J1315.4+1130@t?'Àa"@RYg 5)­À:'ýýûCÀ;×íÂæ™ý¿ÃªM›œÝ@+A҈M—?ÿdï`u‹¿íYo7¿áXwŒÒ½¿ßW.e3?Á?jƒ×e'AGNbcu?ïú$½Br?be¡Äª"ç?6Ís.‰}‹?T?ê;w‡?8QfçbèC?QQ9ºÂm?ïÐþäX¥?yКgÏ×?bI'XïqÏ?iI‰."'?l·‰·èö?qlºû<Z?ïryìãË
?|ÐöÃ9•¢?{mýŒYØr?rÂøӓÙN?…ª†àPó?s/{<»É?ïâæÍYñ?j	¢U?f,¯?&Û5ëâ͋?lVɊmT\?iâsp¥·3FGL J1316.0-3338@sL^`=Wy@<ñÁ'°—À8I[	T=À;6jEî÷š?ã˜ÂÁÜö@Bv2aQ)@"ül—¿à*¶Fšæm¿åuµÃ_ªy¿å
H@5¥(¿æîÅ%ñAGNfsrq?ïøzéö?Eeô¦y§?7ÏwcI³?0ÚÕjb›Õ?CÊY?³LÍ?B	Ýw…Æ+?ïÒÔo_'?y¹ˆL~;?a♆£í?eDî7¨?kI[vÚý?s©#kü˜?ïAç·ê;Ë?†yC7t?~*ý¿×u?sÛÎ÷Íkr?8I½ˆ¸?¯_磑‰?ï⣉uoG?rëåY?êeŽôZ ? ?é¡V½?lÍ#^ô?rËnWÕÎg3FGL J1317.8+3429@UÀ4 -œñ@T-€/eHÀ:7m¾I|KÀ;ñò';×?ÊLNöeÕû@›ôgÆc@«Jàxü¿å(­Q÷x¿èYV¥ÿª¿á_«ÀHì¿ïÿ¸JÅÝ+AGNfsrq?ï µ5æ?¾G¯®ÏÑe?G~kç1¬?dô‹¢›?›ÿù=ä÷?¾ìÂþ»Ò?ï?Éå—E©?šÙ˜ìWªP?ðFaíƒç?…Üä|¹xH?Ž@8AÁ?˜d4ƒ|?y <¿? ¾ûT>·?kýX÷Ÿ?u´ÍºžýÏ?£+i¾LU? ™ç]B?ï!ë;WÆ?"CQdv/k?^ Ã#ÛV?ˆ'řBj	?'r7©?*]Ʉ3FGL J1318.7-1232@s"¿Ÿ‡ð$@HãÓ %¤ÕÀ9³ '²ÌÀ;¨—¤¹¿ï'Ž>;@™íÎ à@ǹà`þH¿äkB	K‹¿ä¼0LÎ嬿æÃq¦­Ì¿áÓÞTð®eAGNbcu?ïí
`Ƨ?a)÷:'{?E}¿ •¥?C¿™¥¸Ò?[,ë³"f1?]SÐmPp?ïÌHƒ¬]F?y÷Fy?gôƒKøóÝ?o«•#k½?kÂù©ÆL?pºü=Åàò?ïe©]Š?óz3ð)M?xû±$Œb?p»ÞG]à?Š@'å–WH?wpÃûX9À?ï¬Êt·ýr?zïÙßNV®?8wçà]a?>(ÿÏJ9?"	£'ý»?z¢šˆ<¯3FGL J1319.3+1402@t¬–ÿÁß@RØû_ò®ßÀ:Նjè¬&À;ýŌf«0?ãPŒ~^ú@H§Ž¤É?ý؜žÜ¤†¿é•Øa€x‹¿Ùï38'—¿ÙDh(¢$q¿Õ¤ýä$Š×AGNbll?ï×\å.bº?¬³íWìw?q'èB0>u?¬±žm«Q'?IM)4ó$ß?bgaª`45?ï~áczF7?'!×W­?E"E/,ú?‡«'Òͤ?€¤ÜþÖ۝?'m1¿™›Ä?ï0M+µò‹?…tçœw…G?†~Š"¡aå?{Phå?n*ïáûX?~MJ3j\Ë?îݛŸ_¾<?šwKÑ>ü?ŒÜ¸"'U?'£Øï‰1‹?•Þ/Ñ¿
ì?"'AÆ{ò3FGL J1319.6+7759@^CE€<ÑB@Cƒq_¾¬yÀ:2ÂfA}yÀ;äÚÔÍLO¿‰9	`üÅ
@—½Clç4?ü'_øc)¿äé»Qп×w3£E"à¿å²R^OI?²×œù9VAGNbcu?ïè 2×6Ñ?dÙZ?±?W—苇ë?]#jÖË?X'±Æ
rž?W1ËQ©þ?ïÆÝ֛‡â?}71"§`§?g¹G¸^8?iH×=Bs#?p´Ž_à"?w'Î ˜lÏ?ï;¶yË=e?‰8QñÛÆ?†ª§'Ïh5?€ñ¹@šè{?Šgº
a>:?yà߆a"?ïÇW5Þ°?x?#
³ƒ~?BñÕ浃¥?Nß?`[Ý?yöD(9ö¼?w¦Öį3FGL J1321.0+2215@vj¿ß~€9@TlŸëWÒÀ8ÆÄŸäÀ;zŠPPzl?Óô½¨RÖ"@YÌ­ÃJ@_ÄŠŠ¿ã–¤'çã¿æݳ*u…¤¿âÐ1ú+³@¿êïgMä[×AGNfsrq?OèT÷?µj¾%´pQ?I$$B¶õŸ?fBoQJè?‰éÁ¿Rß?µZ34õf?ïÂ	ÑY?")W"=S?g\šL…'?rhºéç­u?sM'QTŠ~?€™I"üŒÆ?î©6ƚÎø?–aÍ*Ö#Õ?†DŽ+t8¬?~ÿnjVÏQ?Ÿ¶àì¯?•4Óàå@Y?ïŸsx—!?'Ýf÷…]k?aáêŠ
Åv?bôì+SI¬?ƒª§Y–ÆK?'2ìÛ3FGL J1321.7+8312@^vÖÿ´@@íÛ L¦¢À9ˆœ×;»˜À;å#ôÑΔ¿úŸ-èE¤$@¿:òð"@"ÿï¿çÿÕJF
¿å[ËÙæC¿ä-"XÐâ¿ìຍZ)AGNfsrq?ïô]R{w?Uþàtˆ&!?LÆ}À(¿Â?N:O"Î28?AÄ8SÕcx?GyãQ#?ïÐZñ—??z<l‹Ir»?bŠ÷òT[?h¼kµ3ί?mþ±‰?s"e'¸9?ïÔÖO•—?*æÌ*?Œðh
½­l?"®D5
O?‹Úba\í?12šäp?ïïL¤Áß?fϤgúD-?aᚧJ"?$""ÙÑ?`ˆ+Ôӂå?f'…ÅD+3FGL J1322.3+0839@t_._ú;›@Qˆ¹`~TÀ9êk#d‰À;ȓ6©	y¿í0ÇA-Øç@5KÈÊà@D_ÖT`¿åªü°•3®¿ææ*cMO¿Ì-Ìnâ¿ïù_'aÁçAGNbcu?ïËÑoúlý?¥vyz¼;?K«
‰'ê²?Yu+›ö?v¡æ±™#@?¥kìŒDƒñ?ïÆTŽ×
?€ic·Ð¾?g­ÇÑq?p€á"ú%1?pþÕy?v?N4%F?î(¡©@Õ?ŸªÙ"î5?¡/ƒöu?—s¦þ;t?˜ßlŸøk?ó0ˆñW?ïÂÜÊâUS?wmë†l½?>ä{Ú<ãµ?K›o"Yí±?|£RÑ1ˆ?v§V"Õö3FGL J1322.6-1619@s›§ÿyÈ@FòÖàL'À:…zþ£ßÀ;´°t§qÉ¿öÁÊóƒÅÈ@
my=¿Î@Ùö X:)¿ãØ_'.¿å‹öº±í¿ä2Äߝ׿äuø»Ï5AGNbcu?îþ1Y–µ?¬¯©òð‡?l²¡"ž?s(À"."9?œ¨Å¤9hY?«¦¿Ú¼ÞT?﷚ùFñ5?…	H(Ç?q"ú²ÛÇ?&zŒÂ?r­ˆ©¬Tà?w¹ƒ›â3??îÞé!ç?–Åà?'ÙM5P?€ÍfÞ¯K?¦Ux6ŸVø?'·LۍË?ïiuìñIw?‰4Nç‡üa?EEBx©[m?Ló~¥'há?''N†@?ˆ½§i#ñ@3FGL J1322.8-0938@s»î²Ñ@J9JÞ™À9ò#žjºÀ;—ÿ'E7?ßÕs順â@½×Zob9@	Ÿ#•¿ç˨÷ý¿åäÁ ØMñ¿ìböuÎÊd¿æ6É5œ!½AGNfsrq?ïû®öãbâ??JÙ$;ï?41x^i­v?3Ï2'Vu"?,­¡þ€m?2·…Xº'Œ?ïȅþß}ç?}N;҇Ó?k/ŦÉn?r4âÄäÐ=?ltÑZÛO?q-#{Î×??ï9rŽO?‰³ê~¿?~¶3	‹Ü?voÌÏÏe?'8d!}s?†UÑӞô?ﬦmëA	?WÏì?_>OÀ¸œ½?aŸÆÒ\?€îšª9?€Ž3Keìæ3FGL J1322.9+0435@t,@FA-@PìŸÐë?À:_nÔÉñPÀ;³gþìډ?é
Ƨ™·w@
¡×ŒÄI?ûÕP~ó{¿ïÿɯ"‹E?ïúK"	¸¿Âá‡é\¿7¿áfŸ*ÀAGNbll?ïò£AWÂ?[<]Wk*?G	ÚÑÜ(?E¿hlÐBÀ?Nj(Äæ´?UÌÇSG§p?î$DÕ×]?´µšÎtå?¤^fx?±™Z^E?'»]:ߐ†?—I9¾î)¬?ïšǃ?ˆF´T.%B?‡=]y½Š?|½òÒ? ~(ƒm?Ã0/'än?ì
˜ÌÉ?µ"jNwrã?º·öÕ	?´î"Nù‡K?"žÔ··È?–~JÇ#3FGL J1323.0+2942@Kš¿¨!@T¦$`1˜ÿÀ9Τ…À;"Å@'H¿ßÄßv%T@.ëí¤^@)KßÒc¿á~ÚxSp7¿àQs.ZË¿å)zûÒQz¿Ù0àí¥AGNbcu?îѵ<²?²U`w?'ôÛLUCS?'4—{¶T?¥">":?°ÂÐJÐø?ïj"M¸t?™á­ãÁÙì?€sˆæ?¨—ÈÞF6?…Ü	÷¼Ë?~ pŒ?ìÿ#?¤Iý쯲?¦³Ë'Û?"+*ÄÆ~"?³®!Sé¦?Ÿ)"Ô™R?î=±­b­q?¡‰Òfë÷Ñ?†L*«&ë€?ÑËðäûS?¦'Ún?ŸfÊò¬8·3FGL J1323.9+1405@tì¿ðEx@RºÅ_ñ_À:1Sϊí.À;Ñ#2ý?ß;¢9¦@¡Û1"x@›·1Ô?ïÿ"77y¿¿Ý^?ðt¶z¿ãA?ØTŒÂ¿Üã?AGNbll?ïñ¡Î7ޑ?`͛›ù?P‰jïÛ=Ä?Wn¯:]F-?Heñ@Ï>'?V}À…Ù²?ï"oŒa,'?‹ø
8¥?uý昷Á?zîl–_t4?ÊS7e<?…OæRÜ=?ï
Cƒ×‰?_¯W?Ží¦?"9a(·Ì?~–˜±ÏH?[Årp³W?í'Ô+),œ?©ÀaóÉÏ?¢&
Šþx?Ÿ·D@ô¾Ì?¤¼¯ÃW7É?¢VUo7«3FGL J1324.0-4330e@sR°€0<@2ú!€ƒHÀ7¯¦Ç…òÀ:4>ª_º{?Ó°ÙpcI@O92¦›`@94¿zSٿ僢k80¿ésr࿕¿ç4ú|»¿çRÌÒ<^'AGNRDG?è•áhŽÒ?Åã+Jýôà?'À;pä?—¨Þ"'Ú¼?ËPzºïÀØ?ÅÉÝdìG?ﻖ1uà?'"ó͝?gÃ?ÉåKí?j•'}òö%?vSG™Òjë?}²‹26÷?ã²™P3?¶™þ²‹î?¹üÓ÷"%?¨vÕÛù˜?ҁgÏ~"?³&ÐÆù"?æmßBtN?¸oÙdÝ?tÈ. Ê:µ?uhÁ_Ì<Ç?ÒÑ Ã{îx?·â»Z¯|3FGL J1325.4-4301@sXA?ÐÐh@3gßÿ¯x(À7oB¸âÀ:ç|8_ÂÞ?ê1M*Þ®@U8âtª@Ÿ¹<:ï¿è:ªmHпèãÊÀŒ¿åÀæøД`¿âwÄËT/`AGNRDG?î—$sS½?¨ç°ü-X?ÐHa¢Ï?¥uö·Ó¯?Ž–Rgõ1N?"‹‹27Ö?éÇ–è Û?ÇÏXÉfs
?À·Ë	áÔÏ?ÁïñS?°W½4÷OŠ?¹n4~&	ƒ?藴AS™?°6ûùÀÔÄ?µÅŒÒy•?£Ûö×Ð*?¾i…¾.Q?¨¦|ÔsŠe?ÙYŒ9Åß?ÁÞdQ‡p?ÈF#Z[3?¿khR!
?ÚєƘ  ?Ã݌7?PŽ3FGL J1326.1+2931@J8ïÝëÙ@TڿԖÆÀ:²/ÍM%MÀ;ѝx]¿ô
%\ÛÎ@…"'|Ç@Ž@?`=-¿Ú˜D¦3l$¿é¿F™cá¿ç‹ø&Ì{?ÊWÍ.Ïÿ»AGNbll?ïà­tºô'?'5öSJ½Á?G´•:9p?P:Gáçé«?ieeö}j?¸Á˝?ïÌè®a÷R?€ð'Þ0w?`ÐLwëôÀ?jÑ9("g#?q#'"\Ú?|ø=Ycà?îµ_ì—Mß?"–Ìñ½Â©?Œ5T€
§ã?">ÑÀµ§Ë?›9X-ïù?®éÁ§Ç4?ïðcñB?0?bå:/E¤Ú>æç-²Mòw>þ;àg×ß?_
O k?bá9z˜|[3FGL J1326.6-5256@sDÊ€à@#!Kãö	À8?ŽîDì™À;}\L11?æ%í‰t¢-@•‹$‹Ðƒ@ùÀ›f"¿åȨͿäʳÎ+пä±m7ˆNæ¿è|¬uAGNbll?ïáºÚ'N?g÷!wäæ[?P<·¨`T?N¬:!öÁ?f&×™û?edåú·6g?ï3ëuPû?ž½¦¼4ýÅ?e¾|Ùâ'×?jœ˜BÛ?–ÊÁÂùŽ•?€âw?
?îSQ"dôu?˜m
jñ{??ŽÌ wKîÄ?ƒÁ6.i҂?£ޛݽ?"c›éy±a?ïÈ#\ë4T?z·Áyï>P?+©‡ÿÄa³?;÷ñ4pù?{Jg³b?zRž"Ïg3FGL J1326.7-4727@sQ§€w‰¤@-÷`¿]xÀ9]5õ…R»À;ZxOœöE?ýèªMñÐ@È?ânÂ?âC`èo?ïþ¤žv¿Ðû÷\ÃOv¿å­Ðrû¿îÂh?"zNOTHERglc?³Nw…‹F?¶*ô$Jã?ítt-#Ê?¶ßƒ*»ÜÌ?pÞ{¹º'?xÎøc2`q?Á¹`á±p?ÄݱÕD'?èÓJ•Eþ?ÇWƒ3×Åü?µóž•Rm)?¸Ö=à¥?Åâ²®6É?°ìq¨…?çùUr#¾Œ?³m"‹Dúê?´oï՞
?¡·Átñ6u?Ç!H°¡ê?»l'÷­u&?æ½3(Zʁ?ÃÏXt«??»Ô8+Èh)?¸Q´;Æ3FGL J1326.8+2211@
o}ÿ_F7@T#kà"êçÀ8¤ðÂuZöÀ;f's"L?õ-wTuM4@"Ëõak€@svënοâî›
²á¿æ¡99mÆ¿è›–ýïܿ璂/‰tLAGNfsrq?ï젚'ó0?]ۇlìw?]öyëvq?ZÅT¯ù?A'pl\Qþ?Bøt£0?ï˜	¯âì?‹œi·N'?tyÄHûy?|LÎéŒ}•?cÆè
å?Œ$@1xÖ?ïq¢L??F=Ùü?Œ˜Û¿O?†§H
 G?ŽæR¼O0ô?ƒ1_¬?Š…?£7å?§?ù»›Ñsã?™äÏ:©»Ð?ŸñŽ'Ýéû?G¹J íÿ3FGL J1327.9+2524@7·_}>@Th—×5ÜÀ:üײÙ܀À;úé¦Ù¿®É÷G")ï@Æç¨pL?úڒ€Ê÷¿ïÌ»N9Ö?å¹Q
ô¿êlMäF?áªÅK#>ôAGNbll?ï#.-¯9?³ÞµDNg?§@­v?žâ*I^'²?‹(³S9E'?² ¥÷—x(?ïƑœ•þð?"íŽmÍóÅ?d±c° ú?qx9Ø®ö?r^q(wî?B¡à+ƒe?î¹½jðg?¬³œ0/'?™Ü€Â=-v?"#Z"ôÍ?¢–#È2bê?— ‰7÷›?ïÖHUoÕ?~†?ßH?fnLªZ?xƒ›õEŠ¾?cICŬ¥?q"<zí3FGL J1328.5-4728@sVž²gÇ@-Ø->ýkÑÀ9=E†SÀ;2îiՇ¿ò³CÛ[@T¸ëC…f?û0ßÞøH|¿ïëâ§)¥?씪¯Ê8¿Ûù)ßCê2¿"uv'EóˆAGNbcu?ïâæñRªT?qdA€ê7Š?FH½53½?Bäqdû#?g‡
~^¯?pŒCà™Ø%?ï¬>\	¯?ò­£
­?dS
'pÜ?z…µºi?·v3nö?‰!k{oò8?î[2՟tV?™l2S4±"?¦oQ`T¸?"yÑr'?¡ùšýXE?•~Íý?ï©<{ç, ?Š¦ÒŽë?.ιçl?9Â÷¨¬[?…8ÍËPÀS?Š‰îÈïL3FGL J1328.9-5607@sBÓ@N¤©@nÔ?²ÈjÀ7`>"E]À:ÅÁ:c©?ü©}å‰N@­ègÝßÅ@sÃ²ñ¿áäŒö·Ç¿å¦ìXáÌ¿æòhElN¿ç?¨ñóš8AGNbcu?﫚!áëƒ?€ë^Àõøâ?`J—ì€?``;ß̑?äá‰ÿd?x«Üð2`?îрG¿Ž?§ê·íT?fý,tÉ?mֈ—ØFþ?¡x(̜º"?§=f}P"6?íQLkÿÏ?¤0"5aÝ?¸$¤×?"xŒJÞk?¬3–íÿ¤?Ÿ'íÄ!?ﱺ}݉ï?†•Œ¦!4??Ò¬ ´Å?Y´ÃõyZ£?''Ë#vµ?†5'DÅ3FGL J1330.0-3818@ss?À	oë@7ð#¶eÀ9´8ù€ŠÀ;u±ƒ›*"?äwɘÃc@
Xâe,@>Úà5à7¿éÇúÇÔ7¿é4ÀÜ©Ž¯¿ïÿ	(®Ü¿æäy<_Š]AGNfsrq?ïuŠ·\U?•;ÛIQŸ¥?‹MëÁGaå?'ߦìÌg7?m=™m†#ü?{Û)ßFP?ë‹ö"|B?Á­ñº«ñ©?ºmkT¬r?½åèa‰QF?¢eÇn`7?¦9Êï²Ï?ì2À¹'¿¬?¤ä€Uï?£´´}ƒ»?"Rb'
K?´Ÿø~À?¡ÑÙ¹?Û!\Ášÿ"?Ãÿ*•I8®?Ø™P)Õ¦?Êg^I´&?ɤÜvUŽ?»Šg¤Šä3FGL J1330.0+4437@YeÊâ°@Q·: þ¡À:V'šx¼ªÀ<¯ÑêC?Þݳ¹DHž@rѹp¤ƒ@4¬¥Q´¿áþØöPÔ¯¿Ð×ͫοá‡À[ØÌ¿ã@	ʦyHAGNbll?ïÈ#cÜñÅ?€×<p°Ã?h¾¦Ðƒ0M?xÄrý!'?oõR‹
…?pÌhÕï?ïP蕅Þ6?"½Vwùž}?†ÙP6&ŠO?‹k
J,GÞ?"ìŠhaçû?†7]QS?îåÏV{#Ø?Ž°ƒÊ_TÔ?µc'ITÓ?"-µ]Xn?"kcovÚ¦?'k³º‰?îa
1@H?—¹".
`?ŸÎ®^¡`{?'M¼YÒkó?"¯û6–{?ê†Swí3FGL J1330.1-7002@s#ý@gÏÀ²mÀ!î'À8ñ'lÀ:óyˆ'!?÷vÏtòÆ1@ã[vsN×@:~äa"ï¿ÝFž<
å¿å$oÅy‹ ¿æÎb("Ú¿å íÅYª°AGNbcu?不½êå?Qœw¾ÆM?JEë×En†?Q¤ñíw?"ñ±ÇÒI§?~'ý&‰
?ï%Ú?bݼ?£]ÑѐÎ?gÏëLâÏ.?vo4¸Ó*?˜Jºªî?¡Œ×·÷L?í¼ZÀ&È? ^Ú%$¥?—U*ãæ>?‹Bée'g?¨¾ŒÊtg?˜ßž@bq"?ïä¦H'Í_?q³¦YÅ?ÕKxÛ¸?/'
«'YP?j³
$>ÙÍ?q‡éž_3O3FGL J1330.5+3023@L­ŸàÛx@T5iÿãzŽÀ:7²€fÃÀ;Þ¬k-v¿Ü E`Ãuq@
P¨ø².@ÌÀÀz&¿é©Æ}Rf)¿åãÀ.XÙ¿â)î`›KK¿ïÿê›ê¬²OTHERcss?ïîß{¡½›?b*Êø>o˜?UáC£Hx?]áèÇôL%?H¿‹kÃ	
?LÈbh•×X?ï]S~?&é?›¤"2* ?~ºwÚë'?—ˆq›LÙ?n¶®½?}ЇpÌ?í.±éÿÅ÷?Ÿ}YÙ°ÿ?«®aç7>ç?šsùw1!_?¡fxÌa¸?ŽØ|Ƀ,?í±ÉW"?§©aЗ×?¦‡öG\¡?¤á­n?œ¼rbFb"?"2|†QS3FGL J1330.6+7002@]"'þKÊÚ@G\ @hÀ:Ì°G[À;êpçɨ¿ø‡ÁªÚµ@íJsk²?ý~©E¿êö5ó›²g¿Ý3"N*ý§¿Õ	'oß¿Öˤ®YMAGNbll?ïý(íþ?S3Ÿ[fÉ?*Ò0[ê²ô?NÈ_y p2?"«Þµ5^L?;yaдš?ïÑUAIïw?vŸÔ¹:Ž?fO_"Ô—b?lLúö¸ra?h[_";ó?m+²Õd«?ïN҉O-?z8~:÷=T?w!M'†?qÆ»†CF?€[Á¶ë¡>?n`-¿Ñ6?ïå'â68ß?fßî†js>ú*¢E݂?2†A{Z?jHȅÀ"â?eÞ̓XÑ
3FGL J1330.9+5201@[>Ùb…U@Pî`/ë€À:{ÛÑLŽNÀ;ôy±œÅž?×í3¸Fán@öÅ&@ýp N¿êœ.Á¬¿ã†6TÈ%À¿ë{䖱Í?Úö'bñ;íAGNbcu?ïÍ4€0å?€fa.¾'?v4ðjÜ?Éjú¿z=?JGª®UŒ8?J™à¬Þ?ïÅùc€•?'_ùÇ^æ?i™)ÖÉÇ	?vU³?p6¹TP'¶?u§ïLë¸<?î·¾*ˆìª?"‰J‰å?•…%:ˆá?¤Ÿœhá˜?"µ‰§áá?€×
v͇?ïÌˏ±?z×`ð	ò§?Q<•
Šq?c€å¥¸Œ?uKRõÝ
è?yfÝC«3FGL J1331.1-1328@sØMŸS @H!ˆô'À9ÂMFðPÀ;GÔX²H½?ì,û¶š0@›3\"ë'@ý‰€qÕZ¿Ñ«óI¿áÙRûGá¿ç%RuÿDz¿îÒÁǜG…AGNbcu?í{o‹Ya"?³š!§¨u?³°QÈo‹?³*ÜW9?]w1Z"?`3k!Õ±E?îВn«9? …"î;?šæ"#Ô:?œÏDñ°Èy?‡Õ«þ
‰P?Š
Ï!p?éۆÇücW?¬›	St7…?ÁMÖ¯
?¨ˆò'ªX?­;OëR?™R…XþN1?éR@N«‹‡?´ª9sJ—Þ?¼wfn€?°Ô)©Mƒò?¹Z†	=5B?§TÛËsÓ3FGL J1331.5+1711@uÀLSâÖ@S΀+3ŠÀ9œÔY‰RÀ;ÁÂv1µ…?ç¯hZSÖ@ڍ°e@žÿµ¿è`ñEcG´¿ê<¢óŠ|¿ØY‡±J÷¿ë¶?0†IuAGNbll?ï›oã
œ?˜ºÊ¶'Ä?sŽô‡6ŸÀ?vÂXÐÛü?~¹öB'v?"Úï§Xž'?íC8OÖ¼"?´y^ž
ë?ªk,Ð.£?¬ÛvDÖg_?¡aN2e"É?¨(záGR?í¹§×P~¾?Õb_?:bƒ
"L?Žö"¥¥¬?¥ÈQIrÉá?"Þ.JO?êÜ> ®Þ?³Ð$)Þ*?¸(T"S~?®&³€­?°õñ¥ûå?¦µþ¤º…Ý3FGL J1331.8+4718@ZDàÚ Ë@QŒÕ£5À9ê¶NÜ&À;úp¨È&?ã¸OO§×@>Âqªa@:ßßùû.¿â"Cׁm¿él®Ž6‰¿çu*ºúÎy¿èëáÁaÅÔAGNfsrq?ïïákÑU€?`õFT&õ¶?P*jjð̲?W[gԈ‹?P½òd5x?Q?;ʬÛë?ï\¾'åš?'Pï_÷¤N?"Ï35Ѥ?†ìúÇ?"Gåtõl?‡&>…ÚB?ï4Ð×½G?ˆ& Š0´‡?ƒn‡–øs÷?)ŠðYw3?‰Ä3:?~øjMTv?î6R60XÂ? 
Á¢Š©ž? mo^Ùô?''hßR´?˜ZÚ|B®?™D6ÖÍ13FGL J1332.0-0508@tـo&)@L!µ'm,À7rá`؇ìÀ:ìZ
7'g@b¶<g[@%8ZåS×@fà‹q¿â†ž²)ªÁ¿ç'EÍó¿ëyÎÎÙ~¿æÚÙë'AGNfsrq?ïÖÜO…ÿ£?t7È3LC?mVê}×Ϧ?qQ0Àá?W™‹øQ"?`?YAÀöê?ïÛ@7¢&?uû¸²¥j?_ËwÄ8á?iU÷‰£â?dÚ{½?k"hÀ?íå'ˆÅ˜? a.zښ[?¢e½q̝ô?—ºZºdNœ?ž"A‹N0?–?;AóÈ?ïó:¯´Ö$?jQNÈ‹Ç?&?îÿS?J¤®«?V®xsÍ ?i8‰áD(|3FGL J1332.6-1256@sãÛ6†¥@HZ3à\÷À8bÒ°+¬À;eä`gI?ä¼èù©#Ð@Å;'þÿ@V&o¼{¿àí)†°¿çøÛPž(¿äÑ~XºE¿ãR—K$…_AGNfsrq?ïíï¸a6?aãÕTã¿M?DéŽé7®É?Kþ¤ª€
?Y«Èh¡½r?\R'#åž?ïÑ-Ó$'?yybúS­?eäO‹"Î5?p;p'Ç¿?híÜõG
ä?o³ùuç`R?îÃã(l‰V?"™çm§ø‹?‡¥xÔЩ¡?æï›E<?›°Þˆ€$?ŽÑҝûï?ï¼ûHb£?çësóÐ?*[—4&#µ?2Öi8ë;†?€Ñ¾µ?€ý†$FØè3FGL J1332.8+2723@Bzòà\̊@T3
ç»À9ÛO
)N®À;꽉b걿ôËvh'¸@;ˆrTÜ%@	4 ›–t¿âÓšj\¿á%$!rk'¿åªøm©?™¿ì­Hœ•¼.AGNfsrq?ï¦)migÉ?¨ßòÀô?x×g`zÿ?•ãf­‹aª?táêÑX?€¬ÿË7t?ïÀà5†¿‰?†¥Ïê
ç#?aG,ùp?m¯óšó°2?w
֙	¿`?…ØØc±?튡e‰? å{ÁÙÓï?£§‰¯Û?"rcFr•C?¤:B¿U?šcÌ«ۄ?ïïúa¼µ?b/"¦k–?)-8òKd?;4é9ð²z?\ٖàÈN?ao>ç3FGL J1333.7+5057@ZÉâ!ȧ¤@P7?úÁÓÀ9PaAcwŸÀ;Çñf	IUÀ"€`¯î@wڿԖÆ@øA?ep¿ãóõ@Œ¿èb+êG9®¿áïZ|ÖÉ¿è(qcDžAGNfsrq?ïü‡¤™7i?:1_â`‹?G{xE…?\¸eŒo?8YëÇ;ÿ¦?8ÿMÇåU?ïَ…µõO?u}¬:Òo<?^Ž+Ó>DH?e\'¥L–Ñ?g*d`kg?n™°cCË?ï][gk›?ƒ]•›m?rݙf<þƒ?kϋy]Zn?:Yqú¹È?€ó9å
?ïû£1Œ£v?H
øu'ó>É
èáã.>çz‡ìcp?AZ.ä'Õ?Hr[XL"3FGL J1335.4-2949@s£àGÓÔ@@
%`ÙRÀ:mOŽ´À;¼Þ&'d¿ßÒkLª'±@iŠ}qð³@_Õ¬˜¥?ݟVg?Õ-¿èjmÜýF'¿ÅxÀtézÇ¿åm›?rAøAGNbll?ïñ£>´²?aâ¢õËv!?/Ú+¤ÆòÆ?/×Ë>ôZ?X¾=#9¿…?`¶äõµ­X?kFâ?€p@å?kÇ¥øKÐA?l*	Õ»'
?s˜g{¶¦Ð?yYÆ}Qe¿?ïA>-ðO?ƒÿ]F}°? ¿Â48ù?rÉ™W?î"iϙ?€ïYè¼´?ïF¹ò$M"?ŽD'?Û?=¢=lł?CV:Ò=Ô?–²8Ç$¨¡?ŽY±¿Õáþ3FGL J1337.6-1257@t_¿ƒ8.@H/öÿ¦=íÀ8Ȃ•ùÀ;G2¼î¥?÷,\Tiº@l"o^Æ@À
2ˆéH¿åCvè@v¿åÍÎ{½Ty¿é>S-¿ãù;tíŠ)AGNfsrq?ïŽ-¬ ³›?©¬k¹"h"?€ò
-¬XŒ?–æz°ÍA?wTM"?Ÿ˜ôvÝ?ïC:‰Ýÿ?•'Q}æ?Œñ	oàw?É`€-&'?'@T¯
¨?"ù¦-{?íÍUw£%? LíPp?¡_î¼¥¯‰?•`zw2?¡ÊÀà=?•µ8Òs?ê´uE'"_?³hYÐ6?µ 9Y?°ì³»ò[¼?µXµ½2û?¬'|¹Ý»3FGL J1338.6-2403@sÉ}sÉ@BÈ?`h¤À9£ó=yÞÀ;¦Ñb§•?҂Ez2¡@¾]c2Y@œGÿsF¿çoP@ñx¿å6ÎDŠã7¿ê,øËG*¿çïs
q`HAGNbcu?ïVÊ¥ ¤A?™4Æ@$Ü?ŒèhøI™?"ÃVï¸U¦?zʀ]½LŒ?èô7ø‡?î®`ávÁ?£+Z¦uø?š¥
8g?œ]Ò-&M?/›³2Dâ?'êGÎæô?à
ì?'Ñ%0ɹ?ñÁ'¥sâ?ÎÕ½˜?›0C>Kè{?Š`ò…—'?ë[êhpv–?«H?û\D²?²ÑÍ<ÃL¾?¥Ê¬AX?²N߸þ–?¢¶üæMû3FGL J1338.9+6532@\Êοìº@InßÜt
À:"H¶R7À<$LaØb,?Ðуüàw@K–ä³s_@(·_þs¿é~+Ž›†%¿ê…ˆ·bò¿ê¼`ºAÛ¿ïû˜Ì·ušAGNfsrq?ï\†KÿBœ?µ9J"Pªž?"ÅQÀo?µ;Ïe›Ü?EFEߝ?Oî¬9¡˜Š?íЖØlì§?©´ÿ¶" O?¨Q24bŒ?¤cwŏ–Ä?•JÀŠ#¦1?–¹¼SŠ'Ô?îp¡"dø•?™ÏÒGÏ? dµ¨ Ž?—©, C?'"d#Ñ?†'Itø¦H?ëdaH'Xÿ?±Ôb"š¨f?½¢U;·K?°
øhÔP,?ŸYM˜æç?™ítç	™3FGL J1339.0+1153@uWŠ?‰'Ë@QÇ€Æ^À9ž}þ2 fÀ;™5<ø®Ó¿Ø{x´û'‡@ªtb¨kÄ?ÿrKl÷¿ÑÙ¸K>~¿ç•èµó¿Ùͳ¥g
Ú¿»û¼WgdAGNbll?ﻧpcZ?~-¨Ü2
?Qs熌°€?L¬ Ó'P?}Ï}f+&–?| á1Òbç?ïǦ2' 8?~;'9 ?hað$"?s·n	è±?p&µ¿]ݔ?r~­Ó,?îÃÍêF`'?¬ŸÙOw…?Š[ˆÈ?|èC=<5›?š"³‰oì,?ˆ¾F
_+?ïu5`+Cå?ˆ¥‰r]¿?7
[P":"?B`Á`[?ý*Ur‹?ˆuaÿ°ß3FGL J1339.8-0133@to׿¤Æ@M"dŸ¼ÉJÀ:$5a
ÜÓÀ;Ƽ楻ç?JQÝÃ@÷«yjúö@À	Às"7¿Þ£j?^ÿ¿æ(wS¯¼¿ê¥Xl~¿ïÿÒ~ù–kAGNfsrq?ïðBŠg5?aGšÍFÓÜ?Vÿžã«Š?\âîÎ?BÏØx›Ò;?G¿_àú?íüøÒ5?­FÞ¶.\E?¦lAb¡?§"ßgå?"¥þ!™ô
?"ûj@¹?îe%{Ê?œZe"ù·?£²+M
^-?"†—8ޙ?—ØÜÁ;ÊB?ŒF
z™.;?èjZëšû?¶³Û÷Ç¥v?É{*'¬ˆ?¶ª
Úۈ?©ìí§;ž-?£×}*‰
3FGL J1340.6+4412@XÀ`#@Qz¾zÀ:'k¢ŠÀ;â;Ñgf?æ«S	@
˨/3Ÿ??þòŽ?žPŽ¿èVŽjø'™¿èè¼J&G¿ß-Ñîäh?®lª‰gAGNbll?ïÛJʺÌÖ?qsCàā?E­û?gO?F¿
 }õÿ?oIï†cP{?p€Ø€òn?ï·Xvÿ'J?ˆAàmœÒ?pÅk5-A?XýÖ@Z?sŽYKf.R?xÓÃ/ètÄ?ï¸ Ûc?‡rLÙʅO?"¤j̯?v…ƒaÃv?"ù)¯…¦?šI:#Š?ïx…ì¾:?">à§R|?cÄKBОì?vkþÉÒh^?Œí¦´J?‰¨­QL—¢3FGL J1340.6-0408@tYæ?šIÃ@LF}À?`À:¨nH²÷À;®Ù1_?Õ«j¿¸¬@Œˆ;Î7[?ÿ³»@³Nw?Û#8¥fŠ¿ÒXlŽÚ´þ¿ãÔӍêí¿âˆe邩ØAGNbcu?ïê­Úîc
?cݺDz$T?R˜4"=× ?Tÿÿ'RŠ?Xü?[†.©Žz?ï'F9?Š?,A-d?€È$–òØ?…5ZUû"?uiÅ+®ýÛ?w|‹hv?ïÂyW4?‹åz×>\µ?c²µ,s?…¾€ó$e?¶é÷yÚ?{g£™?íøØörz?Ÿ¤È9?œ½hتZ?'+\"à'?¢¼›lƒ/?˜È‰€×'s3FGL J1341.0+3955@UÑ¿íÁ9@Re¢åx•À:o±,]VÀ<ØúØy?×'þøn@Ÿß…65F@Th€Z¿èôԏ}¥·¿èÓ¾šžÁ¿ÕQ8i'û¿å|i‰'ÿAGNbll?ïì9Ø,Ü?gW7y{?A$1‰;ލ?O•8±`'<?^û¹‹W?dP¢oB³?ïãmŽ+Â?Š‡´Lž­¥?x?':á3?iSRC?N·þì?'HªDُy?îÛù"
p?ËT–-Î?…‡áöÇn?|‰Â!
ã?™¼Þƒt?Š™"9"Ž5?ï5TŠTuö?'ó
ñN?~jÆUà)\?€gíìÐ&?'º½ù7?ÖúV"3FGL J1341.5+5517@[ú?̞ª@N3·ßÕ¾
À:aLç9`À<úˆ²Â¿Ç½²"¼¶@
s		i
[@ ^š?¿ä1æ×åÛ¿ì¥/`¯‡¿Óƒ¦K6gÏ¿â«}Ww=ØAGNbll?š‹3?³v'­§ô›?zár´ç½Ö?³kµ'¶q\?zǂ}Ò¨ú?ƒ~Jíp1º?ï˜ZåO!?'BH¡~?z¦2ț?‡ê˜[؝"?yïç%§J?€ŠÑ?΋y?îV.é¥åÁ?"‹7»f³u?‹>ëE|µ?~p§J¶$?£ÍV"Bv?ëu¤p¡?ïSöF™®?Œ›i.Râ?`âf§E÷?d܅M±d?"'ýjWá ?ŠÂÃXÎZ"3FGL J1341.9-2053@sèàm"@D8ڿԖÆÀ9˜c8´|À;13~²Ž?ëÊ]ð‡MM@-ÍX7úm@/òä¼®¿ã6¢Âž[Ü¿èý,Ñø¹B¿ê˜5ôâJ¿ïÿxÓ·‰AGNfsrq?ïE ?"ù"U͊?=óÁMÀJ?:-+3Qý?Y=Ï!p­¡?"!d_Ô•?ï¸ès-Ò7?~'ªu´Œ©?p…>s¢ž?pþÞ؀â–?sÅ*£AJ?u2 r¾ÑD?ïÌøå?‹Ÿ‹ÖÔÔ?'ðy¯K'?".°öåD?‹lÊÎh&?~G»xÛH?ïù!ÿîÆ?‰÷ö–^Ð
?qNK	×É.?uÂ×CåÕ?ƒÚ'ûj?†I$Õo¶)3FGL J1342.7+0945@uCoÀL‹Ê@Q5ÅÑqwÀ:a±…H©½À;¿¤àõx¾?ã¤.)wâT@	L˜ Ë<)?ýë8$®¿ïý:]L•?ïàü¬äO¿ã=ô¤"Y¿Ü±z>"AGNbcu?ïóQCh—m?UNöçO£D?Cˆrˆó?CW*ï=‰?O·ië5Ï?Qj˜¯øe®?ç×Á°7 «?Є:ÏGœá?ʹä@W
?Α7p?§Ÿ±k"™?®ÁËI¬PS?ïFaUob?…_$ú
à?ˆs+Ò8 ?z èH%ڂ?'ýì5Å
?|"+økß­?ՀT[Rø?Ȋ•§Ç?äjÒO={Ó?Ê`tyO?š uâ›V)?¡¤{…¹k53FGL J1343.6+5753@[xš^»w:@Lñ€@,?úÀ:ÄNÁ.3À<rãLk¿Â»ëˆÏœá@
ÁRæVáŽ@C1¿j¹‡¿ë&n"å¿ëRf¦¿­L‰×•ä¿¿à¢ø*H¨æAGNfsrq?ïãBIVe?-Ž«k?\
BÓôS[?‹SñRÐS
?]n*@¨I?qˆ ¤þx?ï²wj>©?†É"áߎ?sö†\ðâŸ?€Òp§j?rÍăÏI9?vUW*¿½?î ·¬Öð
?›§Ü
äóh?š…rCƒFo?˜=ÿ&AY? ±ÌÏ\?ìº/€ˆ¤?ï´ÖçQ÷v?}¦Åõ|ë"?@èjň«@?L£/ñ?»¿)˜?|¤,Ã{g3FGL J1344.2-1724@t?Ÿ‡ð$@EՉ?¯BxÀ8ICÝOÒÀ;+ÔÏЍL?÷åKà¤@nŠ§ŽNã?ÿqZÜg¿ÛV×R6Ú¿âÅ¢¦Þ{¡¿âЬkêp¿æ΂&é²AGNfsrq?ïöy"4®?Kzx¾^g??j(m)?9växvB?F–þÊö¿ù?DÊ$ð#?ïÃ
6ƒ¡m?Š¦'œ"?ngí¡°^?sýÁGYS?nŠÛÛGâÏ?r0-ÆfGB?îBRöLªº?žAöEŽ~²?››ÌT,Š?•;ÞûÒôM?œÔâ>¨+?'£R/ú¥ƒ?ïi
h£=$?'¸â	M*@?gºö›å)¢?m°o+ý¼b?Íè07lŽ?'+ÅÌb©l3FGL J1344.5-3655@s©[ߏG0@8½¿jäzÀ:'‰)ßÍ[À;¡µç­ù£¿îjÐ;þD$@
ès(ö@t{ \ÁÍ¿Ûêj3œÜç¿â,¦|+½¿ê\Yf,? ÄNE³aAGNbcu?ﮁ+-"?‡*h'±ã?yXŠ™Í×?'Yž°'N?o5g¿ŸC?sjsV¬ò?ïÍ!aÃoÒ?}"ËÇÁ{?c4×	ˆ<?iš™¦™6?oËie†¦?uƾ¬ª?í³ÛZMLO?ž

ù?¡"3øÚv?"ᤨæ
?£>c`–?Mœèt"?ï¬x†¨À?''ü	¦\Ž? ö('}Ä?43G˱‹º?"ž&þ…é?'Ž¨ûrCã3FGL J1345.1-6224@sQş±á¿ÇõS`œšLÀ7À'°H1ÈÀ:1È\$Ä?óH•$êÆ@Ctà&Ç@É'?_‡¿ÙY4å
å¿çJ'QžX¿è'}Ô¿îßé	Cu¡OTHERspp?…sOÕ¸}¨?€þ‹ó¸«?Þ1>RçG?Ïb2{®$]?à'"¼ªe?ÏHLèÍ1ç?W^$.?mó†eh¸?Õ\'F±?ÅÀó´^0?år"xZ•Y?ÅË/Œ½Î?°>ƒø­‰1?œà¢2Tì?Ö("æ?¶Ÿ]B\nö?âôYBg?·iøúã!¸?¯Û‡ÝŒ? T:G÷3å?ÓoÝ_é?¶¸°d5ºI?äJXûw
˜?¹1ƒ@¥è3FGL J1345.6+4453@WÆ"?@QL`×óÀ7\ahФÀ;|7‰?ô¼
?Ê5@ b¼bÇ@×kŠ½‰¿àš§*s=‡¿åŠÛyŸŠ¿ä¹v?¹¿çwi^WAGNfsrq?ïõBٌ?M
Àú½/ç?>~"¯÷½ö?9žÅy¨ÌÀ?LkãAÓÏz?HxÙVMl%?ïÛ?A€{ ?vgFõÅ2¹?_SÐj'?gÏ~T_øè?e;—Ožf?l"ê^pâÑ?ïAd¿zö?‹û;ג‰?Ò)®nH?{ùàh¼°?Ž£T¦rÔ?"ôE2AJ?ïþ$ø86U?A16¦›>ÀÄ¿Ûh¦!>à,¦~¯]k?-mi},÷Ê?A&{—ú'3FGL J1345.8+0704@u# ¤<@P‰Î€+3ŠÀ9gíO#À;™x'â3?ê·«ZŒ='@øh‹Ô¡@z¥_ö_ÿڑ]ÈÞ¿ã³MŸ<"&¿ç­Dõä"`¿é†e¨Y®AGNfsrq?ïÞNãzÁÈ?g•l¿q £?jž™#Âæ8?dv"T4,?LJ
…íFÌ?Jq·ÖŚ?ïÊS%ŽÔ?-ÚÚS>?jZÞD| W?t4ŌÛéz?kQü-iÓ?qauRƒ?î:BpÞ&|?˜àµ;]ã}? 
šû°‡?"¤>á4c-?˜ƒ–®Cω?‡ÒêUÙ9?¸í Â?"ü·[vá?m({Šå?j¯X
ڌV?'U²â7•Ñ?ƒ:™ãº¼«3FGL J1345.9-3357@sºÎ wm@;ÊÀƒoÀ9Ý7iù˜ÞÀ;°¨YOý¿å$Ú#'Cy@.¯KÝy@ºs 
Ìã¿çvE`Ô£}¿è…ù‡¿ÞLs'·K~¿æ
z'R*AGNbcu?ﲸ'™ÿf?ŒaÃj;•t?I̲weàž?P\Â2?µ2	Èv?‹~I8WS?ï¹[€#`»?~•Ž§7?mŽý'c¾?l‹mZ;Õ;?tŠÁ%@oÈ?xd縶?ï$…ß´"?‹Ö¹â]x»?yݏ=µÐ?ir(bzUI?–äƒz?ˆcØ["àá?ïnʊ½§â?'ÆdÑøà?B=‰eÛB	?AŽkÔDê?'"Â])—?'lCýn3FGL J1346.6-6027@sZýq??ûSA§vÀ8j^IarâÀ:ˆuk¼ç|¿ÖÈ,
=ïé@ƒë²k"@‹C…¶ä¿éªÊ®Ô-¿â7Bvòû‹¿âÐ=õÙá]¿å<'íØáAGNrdg?ÈËc=Œ·?ÄwH*ÇL?ªBç¼ *?°/ÔÄAü?è,C´ÚÐ?ÇԔ#(¥È?Ç×öa»	‰?Ì_b 1D?©¨u#?°x½>XÀ?èyò=	í\?Í sô;Ê?Ô>D$"W?¶©àhyŠû?Àt‰6=šþ?ªcµ@s?áû jO?·_ˁ>aŠ?àUFán¸?Áfë3L0w?"
}1«N|?}Z>ÑC&?ÞµS7È?Á‹fSïÖ
3FGL J1346.9-2958@sÐe`A‰7@?_ð€0<À9»éœç+ôÀ;_šÛ¸øÚ¿é'©jz¥Á@œ¨žoAV?û熿wNÁ?çKÑ Ø8¿áµ¤g¡¿ÏUsã/Bk¿Ö¨xÊ/þAGNbcu?ïèƇÿlë?d¨#•sú?Eóú7¹½?C¾$ÎT±?a¼yr¤Î4?bonO°‰?ïNj NøÝ?{]ïdŒ?h‡¡Õj¯	?nùõ|>3?oí=ۜu?rêÑÓô?îºþ	‹~?'ÌÇîî ?\Ý֑Ü?€<""5?™ñ͚ãGD?ˆÿŒÙÎ?îËç¸Øÿ?•O¤'}Ò?1½â«O®?4öØr°ƒì?£­_r?•=R…û3FGL J1347.6-3754@s°>€8Ÿ"@7¥`/ÁÀ9‡"ßöÀ;l³X‡€'¿ññ­w6@rš²t@ñˆŸ¡EŠ¿ä«‹3؛¿çt½ÛB[¿âû¾ŒdŸ3¿í]0©"âíAGNfsrq?ïéðøòÀ[?hc9%ʇ?Ab?½È?@GÞޘ¹?aÏt¯µa?f+¥©<ë?ïÎJîCï?|rü	®2?aÇԋzÒ&?g¥èY.?oî†A>µ?v•ý ¹&Þ?î´d4ã(?'.‡~¶À"?'H꼫b?†|…
©¼?—3ˆ½[ïÇ?ˆÄ2².?ïØ9yÁºs?zgQKcœ¾?@Sžœ`?$(K¶u'?s˜ÎÔL¹?z]$ip
Á3FGL J1349.6-1133@tNßÒc@HhŒŸ¶MÀ8¶ÐE®À;mÖ£æ#¶?éJ½ŸCÛ@Ûç3€`
@"³Gùi¿ãÒ©p&X¯¿äQª¶2½©¿æúC‰Rà´¿êh)pMJAGNfsrq?ïà±"²Ô¾?j <ÅIíø?g-¼–ÄE?cë•Z¬Ò?PBAnNùÏ?UAš4ä¹c?ïÑÏ݊?y*€¦õûK?g- ¯ó`{?pþ£6Ø©Ì?gÑG/î?låç%dö?'p•?•rr&¾dK?šjNÿ¬Þ?q_R‰?"$lPo‰?ƒì§Л€?ïö>¶'Ì?Y%H§Mñ?
÷À‰&€?.܅A\j?R'ÕàÞ8?X¡ªÒvü53FGL J1350.8+3035@I²Žÿâ£Ï@S#ÏÃøÀ9
˜®¸À;Â^VY?ì÷"úXÔ¶@«[ƒc@ø¿ƒŽ¿ÛPÎWD1¿çŽ8éð7û¿ã5MTÐ'¿êðw2!ÌAGNfsrq?ïòV´@‰"?T­.íK$^?IÇýiÃ?G$'ÀR˜?MžgoëH?Lcq0
w?ïʽÁ?'íá¡N¡ë?b¶Ê†8?j
Õõ¼ ?qF:8é?€Ã&ÿ¤ïù?îƒ_¾_úÙ?–¬ñåo"?˜c"«.?²Ùýèñ?—0t´Uvß?‰ynæûj?ïà	EIÛC?s\'}ûkÆ?Eè3(}Ò¡?J…v[Ô«[?j|­ìJj?r€ÈITÐ3FGL J1351.1+0030@tÛz WŽ\@M⟾vÉÀ9ãÔ;kçÀ;»€õ]县ÁRڅ
@'Â("¯@€Z€ª	~¿åò@òŽ}\¿Ýúê
ò©¿å6èR¿îVÁ(ŒëAGNfsrq?ï—<:\-?¢¹bJ^3!?'õŠû²á?Ÿµor¼?l홷T(?¢%Ã*úû4?ïÓ2nyÌs?y}ô—"Fo?dÔ[nºç´?oÞ°bÊÍö?gù6x¤ç?ny'Xvø?ì($Û€?¨|àÍÈ^?¸À}•ôÂ<?¥Ë` "ý?š9ÊÇ?Œ\§{»?ïæþ¸ô^–?fdyŸ·¿–?A'?c¦?MüºÚ¨Bœ?d·†;¾Î?džhr¯R3FGL J1351.4+1115@u·
?‰'Ë@Q2€	¥›À9rÄÞÁÂÀ;G²'a½?ã£àU§@š0øñBù?û^ƒþý¡?ïõ9µÙ@N¿Ð÷ñ‹"¿ÛuhŒÜF迪ªºaAGNbll?ï»î'C5?€–P*TO
?q"S5Ñã?v´©_o?pt^H?u7«8=}?ïÁcÈeê?}¾ÔxIIo?jڑk,+Ï?r©í»+Kh?qàÓ<6õ
?t9s÷"‰1?î?ÖúÀwÃ?–ž´‰Èt?–JQÀàÀ?ˆ°žNB? Ýgsˆ#Ò?M˒ß@'?íN¡…V•"?ªÅʝHø?Š aÃí?'Žá{øÀâ?²6ñi)j?¨&¡ê÷s3FGL J1351.7-2913@sæ³ S\ž@?ӆ?IÁëÀ9}ÁÕ"äÀ;Œù)L)¤?ÙÃp*"2@ôªaâs@+"¿lçà¿ã¡[òï÷¿åã'*È¿ãÆ_׈¿ìHõV±AGNbcu?ïÚîÞfg"?qü;l?`ª1rZ›?c~7élî?dfð'>f?dE€îM?Ååõ)?†qáp'à?|ٟeñ?wúÕ;bo?}Sýþ Tš?~aÁ{eŒ'?ïgm=•??‰§"úxÆ\?‹ã"zM:>?š2>´Õ?Ž6Muæ?}®ýóSóÄ?'›~—?"æxV ¾ã?ƒý¢+Ï?wdÁ΢x\?¢¥.K†òc?",z
+ê3FGL J1353.1-4414@s§?Õ%@1>c_Jé2À9YÕ£5#ÎÀ;‡ýgŸKŠ?ÝÅÔGaà½@×Nìő@¿P +"¿é‰–Ü"°¿æåÜ+8‰¿ÝìäÅ<	Æ¿é3ѳ]ÝMAGNbll?í¶®"z%~?²"ɁöÊy?œoyŸµ€B?šz;óoÿ?¦]a'è
?¯3:§î?êVÌèN]¦?Á$2nbõ?ºFšD(?³ÄÐôè'x?³;R#xΣ?¸1Ï?ëƒï‰ìš/?¦JI—+د?§ðþ""ݧ?•Jƒgìþ?·èfØ¿¾?¡6Lx:ö?æpSÒÍò½?¶"¸:ùÁf?º£w֝ÍÜ?¬èžô:ªâ?ÈìôÉyN?³£ªÔGÿ3FGL J1353.2+1435@v0":¸c@Qº¿ÖDEÀ9ö†º À;Á¹ã»ü›¿îy­:@Öç,õW@½œÛ½€¿ã.êiž\Õ¿è%ž8uùh¿âr2¹«¿ÞЮ›UÓ¾AGNbll?ïôÙîî‡
?\«B7çÔá?,9´ÚÖ?0d¾f(P?RȚìVR?[«©…Xäæ?ïÎñªTR'?z´kDªô?cÿPUô}i?oø³U‹º}?mU¹Zÿ?rŒêÀ$oü?ï+	GüÁ?Š½¿'«±?|'ÎŒˆƒ?}ÁÞ`w¥$?"{3ÞDg?…aw߅Š?ïÆà®­Lé?xj"8çÞ?)ŠTi¹ùœ?1€Ú;lØ?{ÃV»¬?x:"w'3FGL J1353.5-6640@sP @|ÇÒÀ#7À5º¢À9]ÇËÜÀ;BЉï•?¿˜à«ù@œuÁù	?þ{``½Úì?¶Ú¡Ì˜õZ¿Ó•nË©zý¿à÷†<x4¿Ý'û»¼rüAGNbll?ï€ò:?—(a% 4?ywÄ$Ã$`?u)ø«ÿj?™qð¯dø?•žQV³X?ê]ÈWé´?Æ®-[ñO?•´ÚŸ´ò?7ž²"»a?Ãåh7j?įuµ?ís~
€×?›:ÒvÉ¿†?š³Sâl?‰ìL˟Ì?«n…Z?"oa?ì‡{YT'?›úódfà?z.RuTþ?sÌõŠ‹ð?º!@¦-?›'VòRÌ3FGL J1354.5+3705@RišÀ
F«@RXŸá²7À:|¼A%À;üÔyixj¿±"Jn@
(oxùt@LŸ•Ü÷¿Ü$ÖN*ÛK¿áµ¸r©¿è†ñêR¿ßó(ôy-AGNbll?íøIé?°|ÀT…LÒ? 'Æ,ÎÏ?­Éœ¨j‡?"ý+Ñ®J°?·c*fæ?ïJñÒ¯?›4	‰!Æ?†ÇeôåZ ?'¾–°'a?†µ™N¥ùö?ŽXŸÚ1‡N?í>àЏ?¤Ž`Î0?¤Úq¨n©?œéDÑ«Ó?§DÀWðS?–ù©ì?íúO¿&0?£²Á¹cÿr?¡E¦%æs?žŽÂf?ž*»Ñ2??˜ÐªªöÄ3FGL J1355.0-1044@ts<`Ÿ@HŽ¥?À	pÀ9@'
´©À;†ºö
³¸?ì³Jð"'@'È"ÙÁ@ûÿë2>¿à\ùՐã	¿åÞcK†¿éGl°ØO¿áñ±Òº;iAGNfsrq?ïøÞ´#—¹?Hý4±¢0?Bå°ÞR¥?AÀ/óÏZ?3>ý'!Œ-?@ƒü®h2?ïÐÝ÷ò«?yÙ=/?iTê?õw?sÕMª?f³#@a?kE1ÜQ¾ù?ïð	3"þ?Š!{Hì¹U?‡0yzÙÄS?}ûöà2÷?É ~?ƒ'£¦`L¯?ï¾ô¦Wc?€Ë[-Í~?Lñþ—tl?Uv³i ¡?|çm‹Î=?€aJћHû3FGL J1356.3-4029@sÀüßï¿@@4¹&Ÿ¦ùÔÀ:+qøjàIÀ;®2Ì&°¿áÆ(Ûìz@Y0‹yp@{P@4M¿èî)jª¿â°´ a'¿çÿ'z9ÏQ?Ô6aË÷åªAGNbcu?ïÚù´L±ø?qÙwêvÛ?Y‡þ·¬?]Êìêß×?hBLWÊ0›?l—°dc'b?ïÈéËùћ?ðñO>p?b~ÜT3ïT?h8ïܲö?rK«Øý;
?|Óo¹yTy?ïæ/ŸàK?Šè'*"?‰]éL²õ=?}³hó³´?"Eeª|?€¼æì?ïõµæ"?zǶ&¥™ã?©˜†uä?1Bœ¿%†?}ºÕÂó?z¹¥ŸÇ|3FGL J1356.6-6428@s^-••Àð[ b 1À7ær/ÈEÀ:µ'v©V?ñ+$®¶j@U$Zþ@|'@Y·V¿äOEAÊòú¿é>'úeƒµ¿èyæ¼É/Å¿ëÇѺ66PSRPSR?ÇF%Æ4"?¿ŽZvGñE?Ñváڅ%"?ÇíPÊkì=?ás¡0lU?Ë:VW%?e?ˆyºwå}?©ôÜ £&?ÞN\—ø§–?É
%AY%?ßÙÌ_Ú?ÈçE	Bª?Ñ7!½zDI?¶E…æ'€?ÎèhØI?°o›n.?ßTÕÁQO'?¸páîôÀ?À0¿6P&Y?¥È >?׺>ÆOÀy?·áŸeGÅÚ?à°ÏD-?·8KH®¨3FGL J1357.5+0125@u?€ß×@MæÃ`<€ºÀ:p
TÙÀ;£'wŒ(˜¿ÿ;WýB
'@x_ã@#lYA:¿ézcp½­J¿ß¿üõ‰"y¿çˆ\›Cé¿Ä…âØ|ÙDAGNbll?ïïPÏá¦H?aB;–š?S—][¢¤?X9DµZ/?KŽÂ!¡N?PúJÊ)m?ïר›mêR?wÏ"í?aM
u­?kTwøü–m?g
Yˆ7¿?mÔ£'•à‰?ï,›˜5yÇ?‡Ü#o?‡u]ù|3?~[hz⯴?c»ùžì?z_9I&u¤?ïâ9v—âò?j"€Ÿ.\>ùjÒ8ÀD?Ur0õ!?m"µDxœä?iïߤ´w3FGL J1357.6+7643@]ƒ5Á'ì¯@CâÍÀÓgÀ9Gêz\½À<'ÇÅý?òjêD+þá@ŒgH8¨é@ßs¿jc¡¿åq8b®1¿äÍ$oËë¿á Š.öN¿ï ¯?‰AGNfsrq?ïiȊ™J±?®·7Á•i?Œh{¡³¨Š?®s"ø¤ž?rJÃoóUx?w©þ ?í™éôÕª?²¡U¼¸<(?ªC…íö?­;è­Ø'^?˜;ÞՉ^‡?œÞÊBp?ì0E|C'?¨2l±Š[Û?³}¢DMÑÝ?£6@Cד6? · #3?'ÛƲ­LÑ?í±ß-}¹9?¤AstU?¨õ'"
?œÿ©\Ôoà?—Ù(0¾Ÿ?•ª?ãŽ*3FGL J1359.0+5544@Z  ô×®@Mr /µÐÀ9Nû'²õ‹À;ô4-n¿ð-âPíƒQ@Ïl®)±@½¢À^ÕM¿æI6¦kuU¿ä
"£`¿ëJ.‹>ô¿æ…=å):AGNfsrq?ïø§a]=?OTÖi ©š?C åìC?Fê{Ô÷8?4µË)=‰…??x3·Š?ïÔe
'?xÇF;¥êõ?c¢§Ü$?jªï<-RG?gøNæi[?p_C0!?ï,÷Ӟµ?ˆ©üZ9-?"ì?‡¦GÄ?Yœù–(0?üA]¦AÎ?ïêé}rû?m"½R—(á?4õŸ¹E?Ti±iÛwÇ?c[buÝÁ?k0=}Ãë3FGL J1359.2+0204@u+é>ê!@N矶êÀ:Û/fÀ;"ãiÇC÷¿Áò–‰KT@
éá·?œÎ@©Ýÿ¥G¿q&ʚ˜Î¿äk8>¤šB¿âÊ˲4^ñ¿ïê…¼AGNfsrq?íÖü"è(?·Ÿ½ýä|?¯ú‰-H'}?³¦šLßú+?œðÑØ?¢ÐÊ6'Ñ?îŽ^Ô®Í?£þ<"2c?ž,x0±F»?œgèÉ?­9‹ŸÄ?j…³o\'?éXƒp§?­Lç—@Þ?ÀŠ¼¿é^?§÷](W‹?´'Òbd¨?¡B
?Yd?ê—ý·Ù£…?±#
áà¸?²~Š†´­h?¨ogÜêG×?¸Á‡º~6w?¨I]¯!÷µ3FGL J1359.9-3746@sÙtàM/@7#Z0FðÀ9iÀJÞJ¤À;s&îR{?è–îÞ3kV@Z?A3@0rÀ;ïÅ¿å7šÆ•P4¿æ˜û;A–ñ¿Ôì·p;Ÿ¿ÞPF¼v/AGNbll?'ñMm?‹UT©`ÿá?d	‰å?	?bŽ›†Š¾?ƒwá3U4?‰gªQš)?îõÁî#h'?£ùbê~î?'ˆÃBtƒ?" YxÜ|?59xP†¦?™]½cöØ?î>ÒÊà…?•ô
Orü&?'ø‰wŒ?'±#™m2j?£Ž–téæ?'cpAÜ°?ë=²ÅÍG¨?ª8°(V?"ÃŒŸ¾3?"£êãèþ?ÀÑ6é–?¨!y˜®N3FGL J1400.5-1437@tnݿη‰@Fßä׆À9e=?&À;Š²@YŒc?ñáÐd±ÛZ@
ZMÕ ÛØ@d§ê9?«[ž§~¿á3(N±F'¿äÒõÚ~|¿ïÿK3PSRpsr?±139uRO?µ/µ¿
+?ëš ÎyÖ¸?ÀÐacé$?±ýÆR»÷õ?»ëjDEˆa?ºïŒxct—?ÀS} \ˆ?ëöXsÌ@?ÂßZèx'?©‡üRË?¯R½øÿ?×ÃÞËO?¸1Y³'€–?Þù1Q-_?¹tP¶"´"?†Yx¢?¦úÍâGB?¼A»òš?¬ˆÌ0…4?ê=6¿Ùe?·/ hdò?³DZWùšË?«O¹à‹3FGL J1400.7-5605@sˆ€CR@ïI$À9É÷/væÀ;!€´Ê?ç/þÛgÅ6@èhÜ7xè@ù{ßto>¿ä;v€Çˆ¿èl5†Ži¿ä~ÒJ‡…¿íˆgS\…AGNbcu?ïnÈ©Aš?ŒX'\–?k¨yT)4U?g†CŒ-d?c·håKó?Š¯÷<°?íA66\?µ×›«?'y/V¾•?ƒ0§é3Q?µHvz|?´¾n?íðÙ½Jù?¡B°ÎÍ5?£ŸÃiõâ?'jªó¸)?«!.ú6L—?™økb6S?ìÑÿÿ¿E?¢)zíU…Q?†ÉÉ,Æ?€Ez2ˆC?¶–ÝHáŒ5?¡(ëU7Ëë3FGL J1404.8+6554@[àE€<ÑB@HÇÀgnÀ:"¤?
À<3ÿn	È׿bÓ(iª5m@ªÕ"ð¸9@¿	 g¿¿å•›Jý1ø¿ÝWp3®¿àþówJS$¿åS"ÜôWAGNbll?ïv"œI?¢ŽºÚ՚5?{shIõr?¢Q–2B\?cï–Êf?gdŠ:T™Ý?^'[¨?‡Õ‰«ïï?€ó"ÚMi?OÔ(z±,?y»* ?yF#!Œ?î^Åçñ1ò?£»–å#B?£å¨‹"}&?£¤â~w¨?ˆ·ãÕ¡Žµ?y^À3ëú?ï'#ZO­Y?'ý;ÒÛ÷D?qNû}¬ ?iŽÍHm?'ÏǎUÓ	?7›¸íU–3FGL J1404.8+0401@uuS@N¤©@NØ_¨DÀ9±ŽXó·À;šAÿŽÁ¿þöFÖ~&w@
'ZÀëÃ?ÿ¶MAQY¿åüc«ÿ€\¿à<2m»oW¿×ć^X¥Þ¿å2'#ÒºoAGNbll?ï`(ãE&?—G½X5Ï?k9%ë8m"?kªZ…y?–Ö&0M«?•Èœ-É"?ïºMë¼8¹?ŽHLQ¦%??pV9Í Ë?'9X<a?rгèÔ?}dŒ²?Ýà´ó?"78õ&Î?&°ã€?~âþðe\–? Z…é-¹?Áþ*ú¹?ïnr £Ob?Œ©.
ïtú?7éjÇå?N$×¼LÌU?'ÒC•¼~?Œ@ǃÉPà3FGL J1406.0-2508@t9}sÉ@A[Œ@ÃÀ9¹FMÂ*²À;ƒÈ¸kù?…°ýEÂ@"Mië?þI`½¯ù¿ÃMW<¸ÿ!¿â˜šÿR䇿Æ^,h
L׿äB
s¨fAGNbcu?ï¶Ç0ëjP?'èÐZ¸'$?\b™Ò‰?bo '¼4?}˜Îâäb¢?'Z=8d?ïz%Ý2}&?Š=žCœé?€`9Bv†õ?~KD.øBV?Opê/²?'N=ÔÈB?î<D/?"§êµ±i?±ù¶.÷%?ƒƒÞì>¥˜?ŸfƒAO¢Ý?B-ø'?íÖ°aªòb?œ;ëÉã‡?n»¼OÏã?q˜MKŠ»?°YÏÅîm?›ÄÏ^¸]3FGL J1406.6+1644@É?áAy@QoÄ`Á
À:ž°²ºÒÏÀ;ÅbôÁÞ\¿Þe¼S>&½@ÁÁnSñ?ú[~ Ai?îôÕÄ¿â–û†è¿Ý	º&_˜Ê¿¡ï¢î4¯AGNbll?ï0`z?oÙ=ê/b¸?=èˆÊt»z?=è夫o(?[­l¡Þ
?oH£¼Š)?ïÕJF¦fZ?yɌ—¸?bJnŒˆ?m}p}² Ó?hk7ë
ž»?nŸæˆ+Ð?îã™L£Û?ŠgX®àn7?ŒÑœÔï:Ô?€•'­ÝS?•$%ç
?'ú$ˆ3?ï"#©o«ç?‡Xj°dœ?6'¹´=Âì?B0MéíÖß?Š'‡ÖsÞ?‡ZÄ®ás#3FGL J1407.7-4256@s×àßÞøH@1¯3+¦À9½ø¨ó©°À;˜êË»TÕ¿óDçÈüˆ§@ÖðäJ7@Éd~Û¿â}^â'kÄ¿æ0²
»¿Å%Þ®CM¿ìR€‰ŽoÖAGNbcu?îo'†ŠÄ
?­`qSèšî?ˆ-AIæë?ŠZÿ>ÁA‰?£CÇE®?ª·µÒQÇ?ïZn#áw?Ÿ*08¾}™?v‹ZSù?yt	8oO?Ž\1u'?œãcxí×Í?뀊0a4?©Ð‹îd1?°>£9 ?ÁώMcº?³½
û½CÄ?¢Ë¾Î?î´ç¶4šÎ?¥ß·Î—??FA¾`Lÿ?Sß6^Êþ?¤Y•¼Ñæ?^q$çݹ3FGL J1408.8-0751@tÝ ßÞøH@I'æ@;YrÀ8|«ÆÂǐÀ;SÀ'U'z?ïM,6G@u ,°¸@	ä ¦hµ¿âºp‰ ¿ç-þQ:kr¿åÞ°Á¿äTjõ䕎AGNfsrq?ïò9¨TK?a0¸æ¦?B%•?2x?A4d‰ŽÓ?R‹/ä·Ñ+?\ÑY¥µ'?ï¯éBc—×?'îæ‰õXÇ?uY'É<4?zI ôŸL?r±ÜØè?ucÜ
n?ïNÔ>h<?…á&.‰Š?~AQ(Þ®?wˆc ªäk?*Gævš@?®ˆŸ,oí?î•ô®Ô+?ž×÷Q:?ƒ³Yœò¬? ËÙç©?¡ßH<P°¢?œÿ¢˜sxÉ3FGL J1409.7-6132@sÝàP7P¿±9RŸô¢`À7|[TŠœÀ9±]ïŸ_¬?ð™!ï¾ê6@‡Ý­oº@ïÀ—µ>¿âÜÌG€&¿á£Ó<Ÿæ¿å°å"«s¿ë†}]#PSRPSR?>š¬™¤'?9Äkd̅?Ê`z7ß þ?ÇbRD¤šÕ?éduL?Çf;ñ–Is?A>þ§RŠ?Y.¿¬K+?Òpˆ\©?ÅÕnυÙö?æí!|'×?ÅÚÝ-菩?¨ìq%9?–Ã6‹È¶?Ò¬yw—?´9ÛOK?åüfò&$?´©mÀÉ?ŒçþdNv?óÿ÷pó?Åu·¼)?¶\-(žpÜ?êLFNN|?¹Ÿç÷«þð3FGL J1410.4+2821@DÅk 	ŠÃ@R4¿û-2À:IÚÓöÀ;滵MTG¿÷ÖÞñ'@
‰%Bû?ÿ˜ nJ¿ì¦½!Å2á?±šnHæ\¿ä'ø<‰•¿ÊŠûô$!AGNbll?ïìnÅPc?cŸlY'–?W*Y¼—?_s¡%?OóBêø¥?RӘ¸üD?ïѲêˤ,?yV6¨G>»?b'"öY>à?l­8iШ?kʁ>"Õ?pÔ»ÂG&¤?ï;ß	ï?…á +ûò›?‡sw³lè?xóc	°Œ?'ÞÈCMÂ?Éó.=?ïßôw«è?l_;NÁ*?4Ãòùà?>yÒÑäñ?msuE4öK?kÑ(ïT˜¾3FGL J1412.0+5249@X‡, zû@N  	ö#À: H{™ÔRÀ;ûã±ëŸ÷?åϐé>?@éþ³ú™@L_ª	©¿ædÈÉ\Ï¿ëKúo¿ä¸%3ÒP«?Ɓ¡?Ö.ËAGNbcu?ïî:¦M©?c"ý<•?N7žÒ"Qí?Qk<q6e?Tnãûº'ª?\M"X#û¨?ï´c,<Þj?ˆ'9ª©–¦?td[ÈÊ
?Ò5
b¥?qj_ÈÏ?t7Û'ҋó?îÖí&€?‹ƒ&ûњ?Š(+,í?~ìä%@—£?˜Sšv…â?ƒXJ?ï¢dcz‹?‰L‡`ó?`FkkÞô-?q¢*öJ˜s?ƒULF'ü?†!º›?	Æ3FGL J1413.2-6518@su`4óþÀ8Ô ~$ÉÀ9 ½zIrÀ:ï-؀_6?äI4Þ%‡@Ai×µ@j±€k^¿Ô®<ƒ¾æÛ¿èå*¡¿,ü¿å«ˆ†½Ò¿ã5ގ¿ùAGNsey?äIc0«Ð€?ËÕWCGrÆ?µúdª@ ?¶æË£V¢?Ñî³}ÎÙ?Êe"Í?àò~üÔ(?ÒÑ­~4j,?±Ä"0Ogj?²çè ?Ùª¸5ò}Ö?к6˜AIâ?ä¨8=TzE?·œ0TÀ–À?¸Á)ÆÖ @?¤#P¢ª?ÐE¡ƒe?´.g@ê¶?ãÞì{äÞ+?´­`?æòŸBKW?—x®?Öc·ÞBô?³—ñýló3FGL J1413.4-6205@s…ÿ@O¿çP®-ø6À6WQ'©"À9íi›¥"@+Hˆ"ôF@»¦9:3X?ÿôÀŒÉ¿Îà%¡¥,¿à;5Ý\'¿ãÇÇ)þ3Ö¿ìßØ/wåPSRPSR?Æ˼×|?P¶HÅÅ?¸¼?'§Zó[?²ËºWu?K¼_˜>ûÖlޟ?í?äßÑ ¾?ìÁ*òQ@°?µ/,­Ñ?¹ô먈?µ/ƒÊci?pNA«åõj?kW3hÄ´]?ì-W×⾩?©õØÿ=?½]&+«\?©¨Žâ
]?=ÃeðXç6?>`Þbɜ{?íII:îf
?¥Š3.
1²?µ—òœv¾?¥rš``6Y3FGL J1415.0-1001@tæÿëJ@G׌àM³À:1¨oö2!À;¢\Gÿs?ñÇQ'ºÚ@I O–@I@ô\ mf¿æV*ۏ¢¿ê&J¿éÔ)¯É(¿á»z	äãÍAGNfsrq?î"JC¤…Ç?¥iAg•`?•±<˗?"*íÊò™b?™Å{l£°O?žëíô"u?T»õ?¬ú˜Xš?›©F·?©ŸÐ
ÛÏ?ˆºZ¦uC?Œ!¹kVç?ê·>-ºh?¬ÁMÉûÀ?·âam­?¤eðhÊao?³.,0¡—? …SIo?èæ±N
Þ?½~~ëkS?ÀîòÂá²?¼Ñ(¦"?¸"—ª#L?¬Y EÌ«/3FGL J1415.2+4832@VÖÿÚ@S@Om€6EÀ:9¤$èîÀ<™RKý/?ÒõË'tÚ@çŠizî@Y¿Xš÷¿ìX¬Œîîé¿ã€—.5¿Þø¢æ@ޏ¿é«ÊCZ°AGNbll?ïѕ61+î?ˆ¬ÛTèr
?sW¯ÑB®?‡°,ó_?Pl4Þc—?[zP¤þ"b?ï*4šEHï?™,ę§ú?;l{¢Â0?"¹—,š?"üwh?´?…Šð¹C&?îžR-ÏF?"É»Ô[?C?""m»©ø?‰§"'ü|?˜¢@>œ÷S?ˆ"^,pU?áŠ-ž?—и•¼¥?–¼âF»Ð?R»%|?"'ìst?e×z"è"3FGL J1416.0+1325@) -@P}MÿÒ³—À9·Ät8·À;ÃûkEÉ8¿ä‹×<oûn@°1вŠ@èS`¥1R¿å4—Ö á¿ã2δX¿ãp	Ö©¬¿çˆ\¢d»¹AGNbcu?ïñzã•?`ùšˆ?8¥žp£?6)ႈî?Véñ×:?]—TÏÌù$?ïÊËÚÿ!­?yšï¥z°Ž?fžñp,¥?m_]>­?n•3±­?pçËëëc?ïc!S9Ñ?TM)Lê?x\8•¤?më#Wjé?‹	Žî«9Ï?{î@'FÙ?ï¾ûSø"?tPöke·u?IgD¾;Ö?OñóÙ6?}UrÔëï*?s—Ý Œõ{3FGL J1416.1-2417@th€àe0@AT"¤%À9éé8=^/À;ŠçɨU?ÁJdI£@
ÕQßñ—²?ý¤ã!"ž¿æ´ëQ+Ÿ¿Ôàña׋m¿Ñ¾Ò¬=hʿܱѪAGNbll?ïâEㆿ?lí1ӛ€?P·Ú÷+4?JþÓ"»=_?e²	.ý¬—?h§ä_í?ﯰpLÿû?€^•e?s¤kvëõ?sã¼&í©Õ?tƒ\ce'?v^꟔#?îû̚{~Ñ?Ž·Vfͅ?…zæÛ'Âñ?x }Qh?•ÈùBüDJ?†6q\pu3?îס‰ÞéQ?'òVŒû¸'?ež7f-{f?f>˜Ø¤æ·?¡,뮓;?'|£ÛÚnw3FGL J1417.8+2540@@Âõ`iÍ#@Q§š_ý–™À:@җçè²À;äOªb>¹¿Â>­"@$f@wBIP«ê@O=f'@¿ä=ÆҌÕ;¿ç#HÖ¢Rj¿ÐèyïÊŒ¿Ør%åumÉAGNbll?ïæwbu>¼?k…΍r¸?5ã֌‡I?8kYJo¬¬?fÌ"¹0[x?jc¹²Ù1?ヤ?è#ö?déŸq@²?kýõÆx?tÇaf]Hµ?r¶åŠÈÐ?u5ß9flŽ?ï0¶\^'V?…¾Tzù|¸?°H=þ?rN®žNì•?'ý"d¼äŒ?€‹ÎèÓ-e?ï£Þi›ù
?~lûºÝât?D•â‰PÂW?LqLj"ˆ?…¿pl°F?}ª»Sûþ!3FGL J1418.4-0233@uYO d#–@JÓ`IôÀ8C¾vÈ´9À:§dd-§?óșSù|X@¿¿
œ?òº0»3È/¿«1œÜ]þ¿ÓٖG2L6¿É|µ»ÁÀ¿Úñ3ÉÜžAGNbll?îì+Q_K?²Ó%ʹ?oßá¢ç¼,?|nºiƒör?ž~™ŸÀ¿Q?±Ì—j:?ï"2ǤU?Œ¯ÝúGì?~'ÍðÕ?…áÑ´‰Á_?wd˜`€?{$="8(?è*0`›v?±ÎϽ};?³Ðå)\ãC?¢8tNN¹º?ÅnÍYÏ ‰?¯ŠÄS ?éi¯lŒ&8?´dUä3"5?‹Ûۀlœˆ?Lö·ƒ{?ț"•ÈX?³¶oB	½3FGL J1418.5+3543@O˜XóÖ&@Qe`&±EÀ8Ml+¢E:À;<º¾­OY?ê6©a…"Œ@<cϳ1@w§€)Ú¿á7ñÓdÞ¿áQ<{0wí¿Ý&¤ãu¿åh^©AGNBCU?ïûø,….š?6ØÜk,?+^.è«D¢?&4< ?2"b5…¹?1,01Ú¤®?ïÛ,½	4?u¶ŠýVÇX?\ûà£u–?edŠÔêc/?foQR¥?n€3š÷¾i?ïk羑–9?ƒ‰¶÷9Kû?zdoäáôS?x	||?‡ÓØi)wp?zÕ߉¡òì?ïü8±q1?J¼
J¼Í>Ö¢Ÿf˜pc>ñ)‰_ŒkP?=ßéúT
?Jg®kó3FGL J1418.6-6058@s•òä?À« ƒ¥‰À5ä°S'ˆÀ9m˜‰Ï@>Î 3ý@¶ÓŠ"Õ?þäE,ã¿ÉrÔÚs«¿â"èCî
Ý¿æl@·øvÁ¿ì·ã8ÉöPSRPSR?Ku°—÷sW?Pº"öƒ3ª?å9!ëKv¨?Ñwo ¼1›?ՀQ÷?Ñt¼"'g›?>õÁ–OÕ?X惷¦9?ê—3On ?¾Š¹ES?Ŕ0RAzZ?¾ˆ%Óâd?zð'[
—Ï?{¶F1R`?çÔjŠÃ'?º¸ŸIjÕà?ю"å~N~?º^%"‡´ï?P±U´¡<æ?P÷N"ó®?ádÐ`gI?ÁÒ#µ?Ý%­êJ0?ÁV(u3FGL J1418.9+7731@]@ù?ò^W@CK. &{•À9óË!ÑáàÀ;àƏ›éÖ?êªÑI´)@'œH 'Â?þ€*Ÿæºµ¿èr|Ë$#¿ÖH
y©ÿ¿Û¼^ØÏ¿à¼#p·<AGNbcu?ïò'cšt?_ŸD•ŠÍ7?Sž¶='Y?\%Êtº?@&Ž7
5?>ƒnbd›§?ïmÀ(Ŭ?ŒUEœìî?'Œ'Š»Ò?ö
ÛÑ?'cCý'º?Î¤u­«?ïZÞéê¼þ?‰‡Üw|÷?‡5ZlP
^?ƒºÅÐôOa?'ë¶?vÜ.Û7PF?ï,5_Õ?'>´Q‰^!?"ê+cŸ•e?'«Xñ0o?"…c«ä:µ?ŒÌÑöh3FGL J1419.1-5156@sÆ>KZ@!?" ÔÇÀ99rãLkÀ;¦-?Û¸çV96@
úßڛ—@LÀL
ð¿æKQýE2¿éH<Mtc:¿íù•©
³?¹Éi–AGNbcu?ê.p¡˜ª,?Áöê8þ?±²Š®¿?²Ú~(L•?¼ÙðD{•…?»CZXnjŠ?ìæÏ+Öb?¿âNW= F?Ž·'™Ù-?HZ`LVC?´ò"†æË?»
àDã?è˜Eº
8?±"DÝî?°NúX¿à¾?œ´l~m=G?ÅwlÔ·æÄ?­g}'â¤?è¸'«F©š?¾u'{)Rq?˜g˜íª?¥€±ÏŒ@¤?Êž…ò;å?¾5âéFÿ3FGL J1419.5-0836@u
–Óõ¶@H0%ŸÌ¹'À9ñ|¯~À;~i%]‡›?ópò~$@BwsÔä@)ñŸj¿ÕÐÉöG‰E¿äZÚŒ_¨¿ç4L—wV¿çd^¾/AGNbcu?ï×Úýðýƒ?qõ"ށÐ?p'<T•?pj—¼÷?O[þYi20?Q‰áyP›ð?ï¸2uQX-?T%Ž}?sCÛ$y}?wꎞ5?p£³|/o|?sµJA?í½è¼ùàÕ?ŸƒRÌö8Ø?£c¾ÔqO?•6ïß«´? ¾WqL?"¦Ó2¥·?ïQÒèhØ?'cÈvhÕ?w‰=P›ŽT?vZŸôՑž?Æ§OØ|?šè+¤~Á3FGL J1419.5+0449@uâê@M®Q¿æ4}À:•ža÷À;¾Љð?Ïêé˜_ˆ@
&Î 4?ümá]?ìÅt¾:Z;¿ÔÂ
@ºt¿ä;ÝâÚç?ÔÁš	.ÏAGNbll?ïÜ]2­VÕ?o"t{Iy?Xž@XÓ>Ñ?_ñTVî…?gS­&?ŒŒ?hE¦ý8‰1?ïÐçÖàê?w×|Gl?eû$%õ?lj;kÐk?iÚú¡?oø™$Ö]?î´ùŠR%?'?1,Ïã?"‰†¾g''?†ê3 ?•×Gï?ƒ3¯—UÆ?ït"'PxÃ?'{³Íƒû?a`?Ñ>—H?q1æŠî?ŽŸOw')??'´ú˜D3FGL J1419.8+3819@QlT_Ó¥.@Q³çüÔÀ9˜ov°`…À;ãžs.?ÚÊ4Sf%ñ@
qœ÷GÍ@êÃyíؿݺÈÆáY¿æHÓ¿–i ¿èÀ…tQ¿ãäVpœlªAGNfsrq?ëœMñ?À6»x¼¸?²™}c–,?¯.q.mh]?µ=ÿ3ÂL?¹w''¢?íù6æ'?²T"—¶þ?£¼ì——ú?ªÜœŠ ?™_JÝû¦?žÊ®ô'V¿?ëëjñ\l?¦&¯®ö×?¦õ]ªï.É?"²Bc»Q?µ)ûý…9?¡´BÙwkÆ?è½îÆÈ1‹?»'+I]ú?Ãk§âO*Ý?·+ÝIHÕ?³9: ñ?¯b €h%3FGL J1419.9+5425@X"'`4P@M"ßµ§íÀ9*X R…ßÀ;Õ»¢ç¿À¹u³q˜/@©¤aÒ#@u¼ '+"¿ä%bf_¿å -êÉâã¿áC×ͪ¿äÉâb=ëQAGNbll?ïók7Ø"Ó?VqQ0Ñó?5 i»>?1"¯=WÖö?SÁ‰	ßé¨?TÊe––?ïÂlÖê?èóN?n漅¥v?sëœÇʦ÷?oͬlÉ?r"jyAª?ïU
hÕ?…Ù"?+N~?v™*yÖèj?oþÉÃ?pÁP>?'ôKùnßÖ?ïµ"3õœ?O¶þátW?Kµyʛh?Iœí¾èo?€ÿC¡…ïL?€ËJœi¼R3FGL J1420.0-6048@s˜jŽ:Á?Ìb'KÀ6Œd¤ÅFÇÀ9-#'Õ?öèË°íô@& ß²C@õž_§'¿äø²Ñ‡¿á—~ôt(¿åV+8p'¿ê[õ¡âéPSRPSR?[÷CŽsÎ?]*ÔîZ?À–¿ÿy´ù?ÃÅcÊ´?ëÌT^ZY<?ÃÝ.fÂ3E?j·ƒmîX«?|«ú¼b¢?ÃýEOŒx?¼P½u)$?êå÷(¯Š?¼Ã¡:v4?¦rKÈDN?–™ë~Ñ<?ÒËÛ¼X©Ë?·ã^ç=?å2ípw&×?¸ÐW\z3Ê?Št"'þw?
")•?±õãhV^c?§Gúœ?íWq"¨":?­Cˆ1ðºÆ3FGL J1421.0-1122@tõEߨq¤@Fäq_¾¬yÀ:ï!‹kÀ;¨ñ՚Ѩ?â¥hF‡Æ*@*¦ò—@ƒ{À?˝?ïðHöF¡X¿àKz'°§†¿Ü"ŒM¿é—ðJ'"ÞAGNbcu?ïÏMõ"?yC]'¨?q"ÛËLƔ?užåÄâ?[ÇôèµÀÛ?`"-`£ª?ï[`"H¯›?–r^Ÿå‹?‰×å2Ü]?'ÛE'üI?~¡ªBz_?ƒ\CèË·?ííE§óµ´? ³^%ß©¥?£-–ùn—l?˜î¹]¬*W?›ü¬³?oÁDo&@?í±8n?¥fvu2½?˜:¤»mš?'OÍŽº?¨èb<›h{?¢YTw¤Å3FGL J1422.4+3227@JÅ`Iô@QeæÀ:s¬ ›%À;ÿÀƒé.,¿Ù8Uj'Ï@­¼Åd#@zIŸÜ(à¿ê,‹5¦ú¿áØ:å6ُ¿äoÙ1^¿ïý¤µÎÐÕAGNfsrq?ïqîˆñ@ü?®ê[‹Î§?|ŽE©±?®Þu]/¯Ï?TZ	ÂâúC?[­S¡Ø5?ï)ç´%ۙ?™‰Þ´?‹êIH¥ø?'g£Ng}?‰›ÉÞ@sÔ?T'÷/û?ípå6¹=? ¬Úº?§"ê]ã=.?˜T*¹EäÖ?¡]ÂB.ù?'fVV÷?î£	ׂÎ,?d/GI
s?™(9gÕv?—\á 
V?'œÖ>e?‰®ªiRÚV3FGL J1422.4-6137@s˜^`=Wy¿ä¶ŸÇ±À7¿—02ͳÀ:c""aSØ@ðfôUÒÅ@BŒ:áRk?ñ¦õºgš?ïùÎدs?¸žàLÓºŸ¿Ûæøݽ¿ëk$GSšPSRPSR?aEÉão©ç?g‹Ž¶¶?ì†z
Åÿ"?ÀäùØçœ0?»BB´†Ÿ?ÀÌb€õ	?=åo×X?3S4ñ2å?äÄKw<+?е:†?×Å#—S0«?Ðǔ#¥?œYð¸ùÌ?"íæ†Ãsž?åšþ'+‰S?¸ñ~W¿=ç?Ór]¼?¸G™B¼?'~ ×êÓê?~¶`³é=?êe¾Àr{?¼,Ðê4‡²?ÅCê÷ˆÛ?»a—sÚ3Á3FGL J1422.8-7828@s9(€QÉ÷À0p‡ÀSAÆÀ:VD& }¹À;µü‹×97?ï@"§;@"Õxíҁ@\t_£S­?Í$Ø5¥m&¿ÙÆñ§³Ê¿à\2ce¼¿è)'KãòóAGNfsrq?ï¹Ð¶Ì?…\x=xÔð?qëSx#'p?yÒQ
ê ?q,¬,v|g?vâKÔhÉ?îñIÆ=Ûê?£«þ<Sã9?~¹¢müô÷?f÷ÿÝH?š(^œÅEƒ? ¯LÀÄ°?î?¥×K?šĕ¹23?Ÿ\Kuc»?'[Wœø? öJñ÷?Œ/â*/=¬?í|†C "È?¤Œß×Û2?–µ?U
ô?ýÜ!‡¿?¬ÜüBL.	?¡.ªÑ3FGL J1422.8+5801@Ys´á¼©@K˜Z?çvœÀ:‡ëÚ¯
ŸÀ<!µ±þm?鵡,éu®@
V;Í5¨X@$û_\[ö¿ì¾§:õ|ø¿ì^êв¤F?â/ãu/×ß¿Õg¥<AGNbll?ïæŽ(•¨î?tדV…	Ý?Kÿ x‹U?hV†û9f?bqïL4Rü?mIZUJƒ?ï ÷+ˆu¥?§‡ˆæŸZ?z9ò)ßF×?…ó2ï#¸)?uJxåæ¡?}Ri"š^‡?îÝÔ78˜c?ÐbE¼~Å?}~ÊÐF?†¯°¾|ê•?•†òه‹?"É1äÞÍ?ï'H¥E?µ<7°?TŽ²»óÞ?q"+b§ù?‰<‡—0?Ž;ºdzƒË3FGL J1424.3+0434@uø›@-¹@M1πsÝÀ:…Óé÷€À;Ê(X
Þ¿Øñû	öùÇ@½Ta$X@㽀~•‡¿Ý÷›ä…È¿çñsÛDî¿åh†0ÂQ¿á¼e¦ÍߜAGNbll?ïÀâÖû?€L¢w»a?_Ùï•8?`ü\"¦Fó?w˜v¯°ý0?}=¹"=‡?ï´`ãmԒ?ƒÄºè{q?rß›E­'?xŸžÝeíî?s>®­Ð	i?w¿ú±Io?îz9´%œÄ?'œnWx"€?'b3NYi?†ÉÒ_¹?žVJGþ5?ˆ@×`ۈØ?ï%s6¾ËT?ý[¼ÐÝ?eŒÜ0´AÜ?cuR¿#*?˜Ÿý¢
<?" oò"3FGL J1424.6-6807@swp€0<ÀEÔÀH^À8l›
²áÀ;/*Ê®å?ð>¢ýñ]@{L‹Hóå@I½ 1xÉ¿ã1=¦9÷.¿ç-³;£'Œ¿çÈoè<·8¿ê™¼å¬ :AGNbcu?ïÈÂ=û‹?yguBŽwÙ?húá$è?n n¨°µ ?nç0àài·?mô¢"5d?ëçªîÑQ6?ÀMh_`SA?—Œ¿dHϦ?œ§|*vÜ?ºßx°cBe?¼š·© ?í°I´u?œíxp‡2À? ¨ÃƒT?'Bt\(ت?¤R«¹UW?'¸ÛfÐ?ëf n‹2Ê?­Ë·®¡"?¡‹]N£I?•¢21×Å2?¼;¶Üÿ?¬ÒA>3Õõ3FGL J1424.9+3615@O¼ÿëJ@Qâ (zÀ9]Ô´øš±À;¦V6mzWÀ48éU™@UòŠ÷jZ@ÄÓ_ãëL¿×Gž?È¿å›ÖDg/†¿áaÍm-8¿ÕŒ8ôΖAGNbll?ïÞá@Ð-?l-w9¥Zß?K®ÉR°ÎG?G/¼oõ‰?j3Û&Æ,?izÄ«õß?ïÚq,‹Â?yÊ®3ñUm?XùL[ª'?dXz`ås?i-G1ü?t娮›?8¾"Ï?'Òd™‡?ŽžÐ`ç.þ?…=õ^¡³?™Ýз¹îš?ˆÅþ~Y?ïõ`5wS?`tâáÑؖ>œÌiö+¡Ò>ÇZ™z›«A?UÑrÎqõF?`t‡i6Ë3FGL J1426.2+3402@LÀŸ¡ñW@Q ß@wÏÀ:R¸S™HÀ;áðT'QÌ?ãÅ-žÉ¯6@
SÛ&Éï?þÞ%ÀÕ?Ù¯L+§¤¿ß Ëkg›ß¿ÓeØÍ¿æ2¹˜½|AGNbll?ï±Aƒˆù?'•úælŠ?r¦A7ûëŠ?tŸ 
}O'?tٞ?–ò?yãÆ5¹¡´?î¥]ºßý?¡ÕÆ«Î.}?™¥€ŠŠà?šL£É3ôÕ?'E¨huÍ?"Ÿ•ÜEi?îÍtÁ"ì?ŽJÝûA?š^–Þì?'Bíè=¢?•ÅsP8ƒ¹?Ïx¤Ü?ì}ÍF3É)?ªé€hÿ§½?«ÛJ+hž?£Vå%)~?¬GáqZÎÞ?¡`‰Okÿµ3FGL J1427.0+2347@=}z °P@QúÿåþÍÀ6¡H2ž¸½À:ÁÅìß?é×Pô0¶N@d¬Iõl~?ûŸD®'û¿ÖÝÕL'î¿Üãȗ3ó¿Ú#¹m¬<¿Õ¼aÛ(AGNBLL?íUñvþ?¸ÍìVåE?oöf¢îÒ^?€'ú¶Ä¶S?´PÄG8ao?¸,žûØ»o?ïÑ(}ëÊ?{<·Êt?a®]¿að?jÄBñ#é3?m)$UèÕx?tQÝâ>	?éæá—ò ƒ?³zûڌ??ŒZQDv:6?‹"¾ÏT{I?ƞԋðM?²o¢Íl>?ì^P·p=ù?¯4KøŽ±a?TÌùL§?^´©¸"(e?¼½)ýJ*û?¯­ð«Ù3FGL J1427.6-3305@tRÕàqÅ?@9—3 ¾¼iÀ8'ÖJúÐÀ;[Êò×ùQ¿ÔÚÍÀV‹—@»66ó²@XØ\œ8¿äB2øOÝc¿æ[k2þÚç¿æÍõbµ#¿á|RAAGNbll?ï÷ñ´úF!?NÌ×ەì??6¯î\>X»?E°Ó\£%w?Dá4èÈPì?CÚÚV·V?ïÒ3Å ÷?z¸F½ßÄ?`Ò÷"üc`?dY´yws?lùCZ|É?uðtSδ?ï_Ö½v`â?€Ù¯Ü
¿?vB•c…'?l}à4?Œé¶Ó?|Aô¾B§Ê?ïã(ŠŸÅ†?mŠ+k¿M?™‹¾rfï?0-ó‹ó?l1@°¥?mwîÊMù3FGL J1427.8-3215@tYªK@:W– hUTÀ:apÑ#s£À;±,±8ò¿Ë¯iU•D@¯~瑟$@I¾×ü?ïGΠ·p¿à^–%›Åï¿âž:Ãu`)¿×X
1/¼ AGNbcu?ïè8TŠ'U?aÿ¨'™X`?OsJU²§7?M4Âi2zû?_Õ±À"¶?]|™Ïh?ïžß8<E?ŠÓMŸ¯æ?u¶²üäsŸ?}©ErÿÃ?zÙ°åé'?üí#s"?î·Qѵ‰s?ŽBûKÙÏÅ?'ž"R7zo?…ýóڊ?–w£wW?€@.úp?î)Þ¹$ò¡? ÂF½¿³/?t¶à««Ñ?u¼<¹9¨?ªÒ'›`‹? bvDùÑ3FGL J1427.9-4206@t6m
J@1Cƒ`r0ŸÀ6p`w	LÀ:€®n<ô}?þx"¹7Ē@ ·…gÞa@⾛ܔì¿ßRØȌ¿ãÙù·w·-¿ä±¤0Ëпç«)>gĵAGNFSRQ?�è©Èa?yB
é›ÿ§?Wÿ½.W?\wÿiÑ "?z!_†­?xM¼òn'é?ïƌ
Iû?ƒ8 &{}?_KçS·?dÈæq•*?tøfa »=?€ÿÁÙ
 ½?ëëÍê
ƒP?©;–é»Í?§^y‹(b?›šÓ5‹l­?´òSê&QS?¥sTÅNð]?ïòäÖNç*?l!Á›­©À>ø¤ÏŸ
?$]1®°Q?YÖ8Îó,?l,_ö3FGL J1428.5+4240@S^<Ö_@P93À9KÏf@×À;>vƒêÛ¬À0‹áu%@W]ª*5‰?ù1¶@™MC?Ðm=ú¦=±¿ÐúMƒÁk¿á
a<…í?ÐLW
l¯AGNbll?ïéÖ|‹±?gûpþZ=?J5"éO?JCC¤9Æv?_^	Û¦Ò?e[X#
Ç?ïÜæÝ U?tñð~Ìéæ?[aúä{û«?c_·¤®ý¸?eh$Ë!«â?nI͖¶³?î!{Ðð?mïçœgW?	·îÅB?'ŸFÝ¿?Ÿ(,—Ð?"ÞvÂ'c?ïñ¥1ù(?cc¯ðè>©2Ö¶k–h>ÎýNÅ5ì?\²u²Ù?c…‰È¼3FGL J1429.8-5910@s´à&Eå?õ ¿ÉÙþÀ7(g  ‰xÀ:zõ‹1÷Ê@wÿb÷*@ßaÏÓ½@†Ûw_ˆ¿Ñû@VÿŽ¿ãoÙU¶Ì¿èP]<•e¿ï	‡Q²>PSRPSR?0«XSQú0?1™MÛ¨¢u?ï&ÓËËzV? ¨›¼­¤?šâÙ%Cmn? –ŸIûzÅ?)h ¨ÛÉ?CbÿøÚÀ?ío¢Jd?±‡8ùC?´zNï]Xj?±óå…(?~c…R'¢?tnü~?‰?ìy[1¨¼–?¨ñÎз?ºNîñ*?§çP˜
1?GmËÿ+@?BÌüþj[?îß/APà?'Ì	mü.?¡¯T¾žE–?' ,«'±ö3FGL J1434.1+4203@RÄøä@P^ÀW¦À:4ûŠOzÀ<'~Ê
{¿Ù–Zê%@m÷êï]@"í¨'Ú¿äÐX؉C‹¿ã%8~‡×¿æÖ&'¼¿çF£¦@y AGNfsrq?ïõò°­?Y·Oøòb?D'!©@X?TÂî{ÞÇß?DküX?Eœ+»=Hq?ïÉE·¼ö?z¹&-‰S¾?iw}/»Lç?o…èÐS†?m|=‡½?p*œŒR]µ?ïr\@ÐGX?€ëd¶?{gÌÝÑ?sѓ?ç,Ñ?…è»åàºë?tLSë{?ïÉeÏ>mt?wí1ÜûcE?Tæi—n?V@[M+ž?v}úå+M?vg㉲0ï3FGL J1434.6+6640@[a¿7¸Ô@G±K¹ëÀ:µ´ZæÀ;õãåî¿ð(¿1-Êi@
Rß3›Ž?øCú€º$ª?Ð¥zbò"†¿À»iÝ=â¿ÓIáùR¿Ç7Tºc±AGNbcu?ïî»g<?a€ócÍ?L§›}¹ù?S+Ddˆ4?U֌»r¬Z?ZEnmˆ­?ïс!ŠÞ½?x-ç¸ܟ?fôZ³Ó'?oŒNtXÍ?gŠËmpd?mÑ*È9?îž[×Ä?"vȐ#&?•'Wì^É?¼&$dF?'"ôHo¨{?'3|î©#?ïÞ€ƒ³?jþ<ÿè"U?LSW)3T?&.jÚÜ?pœqÈ?jªâ³çOÔ3FGL J1434.6+1951@5`àЏÐ@PS ÒH7À:0qŒ4VIÀ;q°-YÕ^¿ùu¨6À[@RÆ ‹;@ûõƒ¥¿æj²Y¾¿æ×Îú_¾=¿Ó篧"Y¿êR êNqAGNfsrq?ïÇŌå@Ð?€
: ¢œ?[~6ûîA?aËö,Š¤%?u=«Îd[?zïߕúm?ïÍTøËäy?z}Œ6cn?f[‰‰?kî'Ùä?l£«—ýn?pç€ûuqÖ?íÏï1óãË?ŸQÎX?œN 1+a?1KP|?¤ó吩-š?•bò6—b?ïNښ"j?¼]¸ÿ–‡?.äǨv¶‡?6ÏX-QÔÄ?•æã-¼…a?©ŠÈ‰Ù[3FGL J1435.2+2023@6¬ ŸGX"@PV³`<ÎÀ9µc¾yåÀ;ByÙె¿ñõ[YBœ@
3oЍ@oU ›k¿çž3däå¿æè0-¿Û¡O–U¨¿ïÿ«mâgAGNbll?îD8^M4
?²aŽ% *?È×%?š–jhôp?¤JDS廲?¬â¨à«B?ïOùJ*q?""ˆlÇ¢Î?†äÕø34?‰úû,ðë@?…×}E?‰D÷6?괛È`ì?©Ñ4	wD?±µ¾â*	÷?œû÷&1ß?¸¥bÚÕN¢?¢¹êÿÀÉ?ëØ,€ï8ù?±}s®\PŽ?‡ö†h2c?v
é"?'?¾?Ë7¹1ì?°Þ"˜Hæ3FGL J1436.8+5639@Xp6ßû}º@K'ÿyÈÀ9÷ ·›`À;ì±AV¥?éÜ»¤¨¹@ïçÈ{¯N?ÿÂ\@©õ¿åëÌ´¿ãÈ|µLs¿Öf÷ŒO?j¿ÑPíè®ÞAGNbll?ïÏ·oÔû?­Æ "qŽZ?]aC¢ËO?e|w#´¿d?ˆé¯É§m?­š"«[?,?ïK<]M*?¦¥‰z<?'ÕD·ü?£ÑÞüCÖð?…B¨Å<½w?ŠÜ ÅƒÔ?îиȝãå?Øùš?‹Ž;·¦"
?€CpÍ>ç·?˜!ÉpAU?†tqäʗ²?î'î·L?¥3Öp«Û¾?"0ÉÚwå?š4-â1?£ñ|&Q‹A?œÃÛ»gg3FGL J1436.8+2322@=ÔW?ö@Pzd_ûéÀ9׎¢Å'FÀ;¸"lá«¿ÔxlÀ?9@ï¾v@B½ŸˆF
¿ä*Ic4¿ç-žÂ+Ø¿ãL:'K¹¿à§Á^&sAGNfsrq?ïíkÊہ,?a¿³Všé?*h©¸çã?&íÆFÄ^}?`íªˆþvÂ?a'*¥èï"?ïÐÖIÃÔ=?vn•r9?bÁCDî?h©9æoø?lh¢øæÓÍ?nM÷•h?ï~ÖY«'?|]m÷}€?pÎøM[y?b¹³ÛŽ´ˆ?‡â톊é?w¢Æ¿g$Š?ﮩä&øU?{;'@™«×?C"ÆÌÔó?B‹cìõ­J?ƒF)ÕŠ?zâ8*]^ƒ3FGL J1438.7+3710@OÏ`?Û¸"@PQɀ2WÀ8¬N¡MÃÀ;¤ÖR5W?îÅ9oý@k0¥F@êÆ?iøA¿ã+ñÍ[¿æwè­0­Ð¿â'^³®\Ž¿ì÷=Ûû
AGNfsrq?ïñn—A¸Ý?Uc׀V?KpíU?Eà?ˆ†Ä?O2›‰›ä?Mð¹õQ0?ïÕ¤—O©.?w¶8±Õ"Ö?b--ƒJCÖ?m#Hû/`"?h.;-N?nùa<t?îΌ"Á?'ç§ó²â ?"jž?‰?‡ÚKÐWCé?"+É¿ß?"Ë6Á©ý?ïîþ\ö+¨?h°Oµç²?0E=ÆW½?Fpž?Akž?]ñöÌ7Þ?gה‹C93FGL J1439.2+3931@Q2Ü¿ôw6@P²-LiÀ9ç:Þ"_¦À;Ÿt´*¿üBÊry]@Ѐ:øÏ_?üU«`@‡…?Ê^ɼ–ò¿Úä^ä¼ØŽ¿à†8<B·œ¿Ð›¦G"AGNbll?ïéɦÃég?bbëqԇÍ?P'¡›"?P¶þA³Å?\R/×–4?\|L	p0?ïÜiy™Ý8?tKá[<—?^^ºlB²?f²Ð€¥™
?dg)0o?k=7פ.?îѿĔ»?‹:à÷?'Rn‰CE`?…ïéÓ¬ÏØ?"u˜ä%X?šc›Py?ïÌ:*G^\?wgo¶­µä?³0a5?qýÄq€‰?y²Çuðž?wAŽ¤Xå3FGL J1440.0-3955@tIñQç@2X&NyáÀ:MJ4¸À;¥÷T_Ó¥ÀrƒSÜöæ@
¨Ñò%¡Ð?ýÒ
ÿGv?ïZ–¼
6¿ëê%NÝÍj¿Ù#N§ƒ?R}!$#1AGNbcu?ïÞ¿…@'?}⸞Üù?'–"P¸>?*ˆÿ@Qr?p4k¤u1?}«ÌD¶Ý?ïnID—k©?£oe=ªsÅ?c‰hŽ¶gª?l§wÞè
?‹T¶w|?¢‰Áގè?î·#Dö,‹?ã!7úx?…~ñÝMÒ?wFŸ®yX"?ž\ KǑ?}»g«9?ïÈ©zÀY?znðnÕ>Æcé­u#>âJ²ù¤%?{¨v›B^?zmÛ[Éb¹3FGL J1440.1+4955@UûÐÓ@M•ƒßóðþÀ9¹[O7À;ó¼w¯d?Õx æ³"@c0¦æß@Ð^à
AL¿çuµòžK8¿è®€9²d}¿å åõ"¿Ü+µ×NJAGNbll?ïàõèjÊÙ?r¦9sïŠ?_T¶à=Tö?eN¥D??^¿xJ,ù_?h:`xŽ ?ïŠ:¤z	_?'Zvr¬,?mErI?†l¯­r?{u¨}ˆ²Ý?€ä¾³W ?îÚë…Èê¦?ŽZ¥òD"ÿ?‡øꊤ ?}Ý¢_~ò?˜¦dl?†
"–7«?îžv	j?¡.àKñ{Ü?Œÿõӗ€ ?—Ó7°Š?±Cèñ_G?›&¡ðtTÄ3FGL J1440.2-1538@uÃ?…Q
@Cßcߣi&À9§%?TªÀ;ÔCéd?ÔGÈÛ?p@¤BQ3Na@¾@—õ«¿ÐÆqO3Ö¿étÖޕïb¿å _ƒÉ"É¿âÑ,¾'ÅAGNbll?ïì˨ÍýÒ?_X®Y7n€?Hý¶rC?HŠÛL#Ö?ZZ/‰%9?[à-Ï?ï¤>+!?'Š%¦zA?w>h˜H–ø?vjÍZºô-?v´xR'Øà?xGþÁO*.?îö
À$¼?Œ¤:z…
7?‰›oBT?€AkÒ[#?"rG#îÇ=?ƒö®¸É(O?î:Øf¯Øn?š3*úï•?{€ƒZ[6?u–Rmƒb?¨âi)·\?™Ðç²*ì3FGL J1440.4-3845@tR̟¶M@3ZŽà3·À9ÔuðG%XÀ;gš'Í¥:?±Â™¾¾¨X@Úf¸ñ£œ?û±^ûãç¿ïÏ	XU?æ[éö±Ö/¿ãè_ zù¿¥{1‹a·AGNbll?ïÕG:ù?s@Ãên·?X*£0)O?X"1öœÙz?n°0›ÖóD?n—úä$?ïÅd8
³?4Áxë¸?hB…ðÅ0?pÚsÇÏ`F?q,°k˜?xh!F
‰.?îá_Ø5€ž?¸)¸án'?Œ©/ÜHøC?'§Çß1y?•m+p=?'Ô(@Œ`m?ïct6˲F?"×2iü8?rPš(ˆæp?z‰™'˜pñ?ú¥8Îú®?‰…0zá3FGL J1440.9+0610@vq[«–ò@LKT´FÀ9<¦9»±À;–g¼§»›?á¦9xzBÅ@Ý¡ejè×@úEà4Ä¿æG®)ôp*¿åYø/|¿ßu`Ôí¿Ø–Lgâ'\AGNbll?ïú´íÉ|	?CA†–äW-?"Ás•Þ?˜Íãƒ4á?@|ý*a®?A‡uL»rÊ?ïÆ1pž‹K?|M=Gî?lðù(˜½6?r"óUý?lݖ8Ûöû?nÿ¡"ïL?ïtc2ý.R?~ÒÆa¥'?sƒ—{õ¸?gDíÙ]«?‰%­töp{?yœo<¾ÃH?ï…7pFF?… Ò'<Ã?U&¸.½´Í?ZŠnʨºj?Œ
Lö·Þ?…*܀âGæ3FGL J1441.5-5955c@sÅ>€8Ÿ"?¨{϶ŸQÀ8j3àØŒÀ:5é$h;?ñâãd"Ó@…ÝÞÂî}@x*.¤¿á£º"ˬ;¿ß_[61•¿áû Ôvd¿ç/z¬nˆtOTHERspp$?‡4¸ZY ?‡¦™G?£Åõ@Ì<g?¬¾õä¼Üô?îg_ÙÒÕ?®Ôr™À±9?'ȏ`†=y?£qˎò_¥?·Æ©Aï¢Ó?°ÿ4§Œ÷Ù?ìpæ\½Ù¸?´Íi'º=?Âa™,›
è?¥Æ'½Y|û?Á
KÄ3¯³?¤û>mØZ*?ç$FÃÌPš?®/.ÖÐtß?ɪhœ¹Ô?»æ_Ã??±Ç…í¨y?¡&ܕF"?熤¨#М?¾4€Ó]ƒE3FGL J1442.0+4348@SC8€®@Oû¿ÿ^ðÀ:R@|ÇÑ»À;سc$"?ìȨƒu@
µ2g±??üyvèÀ¿íÖÚâå?¼Ñt|S¸¿­).ˆª¿ÝØÓ+ò³MAGNbll?ïâW(ãx?lÿµ•7X?bÉ<g²F?dßàzz?U¿5û#¬‰?\óÕ3€5w?ïTÒ痓i?ž\Ud)c?‰í
ïpûÙ?˜Î=ž¸S?€Þ8*ª)ù?'z!hÐn?îi*Ò ô?—v깁û©?—úRR²Ÿ?‹Ù-§"·?šàSiKB?Œû3BRï?îžy»ô?žõ¯j»@?"Ó!ê˜
?—–ä_Î?"uxÝég?'4{¡bR3FGL J1442.6+5156@V· '½´@LÌûÆnåÀ:ÙPÑÑÀ<™‡ûâd?åG»ÞgÿÄ@
q¯ 5w?þ–?ïX¿ïýÓٗœ¥?ïÂpdÞÁ¿ÐͰý뚿ê8Te†(AGNrdg?ëéy6Ïeg?ÁÏø/Àã?¾Õ|uRýµ?Á¦Ä›'žR?}ëCq4?–¡uçW,?â7ìúã»V?Òn¢RK?ØW 'e{?Ñòìíý÷?©Ä+Ƙr^?±v°A}U?ë´ÓtÍwY?¯C…6b#?¸Âè¨Ò.Ó?¬Ø^Åjâ?£,÷a",×?"-ÿÉñ~?äÃuó¤ú³?Éb"¤:r?Õ¿«Lꨗ?É7ïD'2z?‡-yl@S?Š`Ayª3FGL J1442.8+1200@ ¸G '¨;@MéšÑVŸÀ9±Ú/‹ÞÆÀ;|1u¿ãy:M¦ƒ@^ŠPPzl?üºlà¨÷°¿çyqcªÌ¿ÛvI³ç¿Ä\qî¸b¿Ý¼ü'.¸AGNbll?ïõ¤Ã±«l?QŬÈÍ]À?:´½ ÿ~z?6Õp—V]j?L'¨Ò"Å?M"¿á'šñ?ï̟t}˜?yr(úÚ?hã°¬qÍ?nh]ªtý?kP~ÚÕö³?p'²«âž?ïiaô*'ñ?€>½ž_P'?{²—é]á?q¡˜RF6™?‡Î7¬Rö?uÂÚêp?ï{tî?‰?"{B 'WL?/é.Æhø?4ý×+³ß?Saïڂ?"M[,Ó\3FGL J1443.9+2502@AKy@]¾!@P,rßñl¿À9D–¸=ɏÀ;š÷Ÿnd¿â/	Ì@ø¯.+aƒ@V¾|'¿àEËE…'ž¿æ(>Yú?¿Ô!Ë4yã¿èKŽÿaÊAGNfsrq?ï¢S»ÛÆä?Žu‰pv`?fá?]ª/?hð+KjQ?å¹6܈?‹›\7®?ï7µFB²Ú?š5y]n	?‰^ï'IX%?Žž7û™â?ˆ³¾Þ	ñ?ˆT,Y?íÌÏë+¸ž?šò»ì™
?•}b/E'?‡ðg,?¨tz,Ó[?–<ÅfJK'?îúCËZH? 5ñ	ïéB?xs_Ý	?y''Ÿg#R?«ø—gß?žÝÍ
B%ª3FGL J1444.0-3907@tZàP7P@2¸ßh°ÄÀ7ó¢²G‰À:¶³žþ]i?ñß°	´A@æˆ*?üùë`á—4¿ÞAPb#¿ÖNÏA­Z¨¿×`·-†Ô¿ÙÚX³5€AGNbll?쾿ìdj¿?±ï¹-}—*? ›·‰ó‹?š½ùC!íÞ?±¼vÁ°<?¯sPŒ?î6Ö ¥?ªuñηˆ?Ÿ>ðƒ-?œûa2'
Ô?™æLªæÛA?¡ìFœ^±­?ç°Ï×ÁG?²¦vI‹G?´ÆÝõQvS?¢›"ÁZÕ·?ÆÙQ¦QG¸?­ÆàCxë?áNF§ï8à?¶"ÅäÞÐ?°œJ?¬ÂyK­?Ù^Ë©á‡p?µHiKÑÅ3FGL J1445.0-0328@uÓ1ŸŒ¨@HuËCòžÀ9§ËtÝøÀ;p	{¸¿îÚœ"ê@,"+ž>o?ÿIØÿ5)Ø¿á,š¾ÃÛÉ¿Ù0õÿ~®d¿áºì¶)м¿ÖæÏ7—OAGNbll?ïä'ö•ÂY?iō±"C?Ug©àþ˜?X$sS¾?`ßՕM(ë?bäzkЈÈ?ïÌ«Ú8$R?|"\|Dž?jO}½w5?u†WSXšA?i¨
d"œ?n&Uñ'?ï3oxŽ?‡IâtåN?‡üUÉ'>
?{¹¨ܲ÷?'Ûg,Z Ü?~ñüg9âò?ï't/c?.ô<§Ïj?/Ei:Ô?2|ï™\3`?‹%ßñÂ1M?E»ßª3FGL J1446.1-1628@u,ù jn3@C$CÀI0ËÀ9á·äkOÀ;†­âü¹ú¿ìùËVÒ@¾…Mi@ßy_'a¿èA5Ø)!¿ã†È1:=F¿âÛåÍ¿æªÔͦ^AGNbll?ï3JæÇ"T?žºox»?h#°Ìœ?gy
¯¬?–'-$i›Í?œŒkžH??ï³}ËÇ?€Ý<¸¸?q"o!8Ëo?qÎд¡ï?tãÑùBя?zgž–u£?îaAò­Ø?—oG˜ÅÂ?Bž¨H?±È%²?"?¡Ê'!ºg?'Œ	"b"?ï	s"‰=?‡*?0¦?U§´ø´ðˆ?UÏ9ÿÏÚ?w/ɀ?Žçp¤A‹Ï3FGL J1446.6-4701@t(Óõ¶@&ÓÈß'·À9äþú2À;]Ê÷àvÎ?ïû¶' µ@xߥA˜|@bÏߦÄ%¿ê Ð]â¡¿Ô+ÿÊrvâ¿äg=› ¿ïþ¤&Kª_PSRPSR@?æèd!?Țí\HPÄ?Ó$;a^$?ÈiP‰ùç^?Š»~zË÷­?ˆGØVšµj?Ø#&'uV™?ÊWRđ›M?Úå[– "?È2þ+~È?Éï"#éŒ?Äh_'½JX?å'v› å?³Í)‹úó…?Î+PŒ.Ä?°%i~.U"?·«%àzC?¡wkm¢Ä+?ÜSØ;«?ºÁ2RU?ۀ–f ?¿ù…[ÏÒ?ÀÐ,D½Ài?«3
ygg—3FGL J1446.8-1831@u••:@B:)@k*À:q?8$4À;›Ÿç't1?ãU4%‡µ'@
¯–§w?û'#¾Ì#?߬$Éì{F¿ï'Hˇ
·?î¦ïc"¿Ó±²ÚÞ2{AGNbcu?ïßsÉõX•?sY•*Œ?2À6P?ÊK?6$G/Ñ?n4/@Ÿq^?s	½±¨¢j?ïm˜5Bß?¥Ãhƕz?'rqŒºŠt?')ƔbP,?''ˆeô½œ?¡ì°Ïe@?­rǤ?\Üs¨?†Ð/ËÄ5?xóê˜ï¨v?žJâ9Á)‰?+³þ6r?ìÀ2Ãly–?À"2¼&?]Á¢Ñ0B?~C?±€qg?¹‡e'î‰?À)J
‡Ë3FGL J1448.0+3608@N"ˆ?Õ%@OÛ¿[o'À8߉çtî¿À;;Ɨ(¦?Ø9scÏÞ$@×vôÓý?ý%ßbц¿Öã"8'þf¿Ùïw`x‡¿ÙAúÚ.è©¿ÕñÆOÖAGNbll?ïüX{Li|?:	R¥E¹è?$§j[¿Å?'ååŒ?2èpnԗf?30a¹˜j?ïÑ_äX‡?y0ÚJ©ÏÇ?cњÛÎî¶?kùHŽ€?jÎ€Ì Š??pèò(ø?ïRe×'?"½´ñ?€¾çˆy?y?w.y¥¹ï?Š§ØŶß?}Da_íÝ?ïQ4ô¾S?ˆqȞ¬Z?Sž^õô‹j?V¸k×N¿?"Ÿ{|èìù?‡ÕLþ#î3FGL J1450.4+0911@ lŸædÎ@LUÁ HàDÀ9íþu¼D¿À;»˜õ.릿éFïþ€#@
Ç+Î@ʽ`s2R¿æ°²ë$P¿ßt ×·¢¿Þ}®±Ù¬Y¿ì6ʸ(-¤AGNfsrq?ï©f¶`ù:?‡€ùæíoª?ùˆë0?ƒÉÿùýo?]fKåÜ7?kl'º¶ÝÉ?ïÇJ¼¾¶?|¸¦0ç1Ò?ktåõ?qFÂ+}†X?m³"%"dÄ?qÃjw©	?í™Ö,"Ü|? 4<o~×?ªÆ,/ùy?›¤]JÎ?—8â'}•?ˆÀ©Ò'SP?ï±â_–ú?|·³œß'ô?N¿£¹àŒ?O¦Ë÷˜¾N?¦\ ?cP?{©p4§J¾3FGL J1450.9+5200@VGŸõÔ-@LF{ÓöÀ9Á
Ìq]:À;¿bÀ¿xP?ða#""@7_a@k=ŸrÌ{?ïåq Ã^¿æ>Ölá¿à.Έ°=¿èŒÚWéÀAGNbll?ì±ܲ?²Ö¾´8-?¨‡ß[õþ®?¢üs3ùÆ?¬fÂ×Þàû?ª¨£ãý?è4Ry¯?Ɗû†æd&?ɕ¨ÖÓô–?ÄñÎX¢Jý?¦d3²µ?¥Ži'?ê%
.?¬ß>#æÚæ?·+Vq–?¤gÞÁN‰?´Ë=€Þ?Ÿr|SԚ?à4Ù±Ýÿ?ÁÁoÐ*?×nw
Ÿ?ÀÊ&¿:à'?ÀPŠJmàw?¶_À8W3FGL J1451.2+6355@Yæœýç!@H;ô|ôÀ:ÌVô›¼À<,SÐa¬Ã?Ï+$]¤Ã;@ÿ˜_ݶ)?þ°Á(~Ï¿í‡t[¥ ¿ÅíF挎¿ä¶ˆî¦'¿ÎùƒÆëÙ¥AGNbll?ï~ô`Å9?Ð|>¾k3?‰ÖV®û¼?›"šÑT¼?i²G¶~ÖË?zÌMÕ-,¯?ï‰îéEÖ?Ž	d$w`?€ûœáÔR?…j¸§/m.?yˆPe™l»?{¹¿@8nÆ?î+XΈ%‰?èYâÉ¡ƒ?¡¤ÀZ*wŽ?›qÂ>è| ?—Kez¦_Ì?‰¡ÊâÀë?ïpGHéˆ?Šî×;ÊÖ?|^P—-*í?ŠQ´²?…¾÷b/ê?ƒ:''
$3FGL J1454.0+1622@2Œqà,l@MÖû¿ÿ^ðÀ9øNz·VCÀ;ÊmÍÓ?¢]‰3ue@@ם¶3Ù@¿‰ÿ¯~¿ä!¶"F摿螓è:ø‹¿äNþC^Ç¿ïÿïÛ*ï©AGNfsrq?k˜,t?™[w
¬è?`"-'R<?k‹"Rg,ó?…9ž«3?—yÏàÅ?ï%Ek;Vo?–Ï&yør?±ÐD<»?Ž(¾ß?†üÕæ'Ÿ?ˆ9)wd†Š?íYLî×F°?¥"8$Í?¢xìÔ?•ÎÉg³Š?¨L¸&ŠÀñ?¡wméËF?íÆ>`[×y?¡¸Ê<\åš?Ÿr248A?•=L§"?£ãð¨lR?›y|ºº¯3FGL J1454.2-3751@t'Ž wm@2ìïÔ;VÀ9R¤ÅFƎÀ;qÆ:âT¿ò7wÀÖÊR@ks]oǹ@ Û´¿ç6üºavy¿è×{È´uy¿îs€Wÿ}¿ÉYSæ(ŠÛAGNfsrq?ïë5ðm?e´;cÁ?Zá½_\?aÑ׺$A?O·hI€
Ñ?Ppu±žÞ%?︀äè?Šp|C¨??cu1ØL)Å?p¨£M6io?zZ!Ðvø?…—ÒÏñüŽ?îÓ+¢ü7?'%}ØÏ?‡¶ˆï®st?‡qLcùV?™Ã6É?D?Œ—ҍ†˜Ñ?ïuK¸Ò?Ù¤Z<ì?.ToèÎ	A?:ý¤.ÝÛ%?'!m©"?ÚǯãcÐ3FGL J1454.5+5124@Uêx $Î@L9o¿«|À8W!CF¦­À;IŸß-øa?ð¶zӅΌ@»W";Œ@«¯‰øè¿ße5x÷|¿âBÿ÷æ¿áï'Á;§ª¿áì6CmAGNbll?ïúÑa9åÞ?A÷LÙw?2Kõµo?1b¥"Ù­¢?6åväÛVç?7k‡Š?ï–sž\;?‡núS	'?{äU'Q#?€Öðé.Zø?xáÛ?c'—?xʔð>Ú­?îõIè?'d(¹oã?Š›&3Ä?"æ"AŠ-?"4÷©6?‰.d¶?íÖ.)Šâö?¥IJºû?'dü¬@?À°yc?©"êèû°¨?£Õoßr‡3FGL J1457.4-3539@tž5 ÝD@4‰4ŸCý†À7he²â?üÀ:ç·I­Èü?úMÔ§6»(@D}Ä&
+@\'eîqb¿à
´5Òñ¿å'Úák
¿äã\C«Y¿è'Ÿ5ÁOAGNFSRQ?ïê‡ÊSâ?gq«äÐ
Œ?YÈÒ18_?c)ý3Û·?QÝ¢†
¦Ê?Y¨äWPä*?ïÐdR5þ?|1rÒچ?a4Ýô‰Ê?fo'3À¬a?ngBÏÕw×?w…â}ñ?îÐà/ܒ?•MSVI?ß(û®¸5?Œßë"<§Õ?•Ñ µµ^?‹îOG'?ïôõÍŒé?b
g¾´~>û=×û)ž?ˆLj}j?U§nbùˆ¬?aènñQÏI3FGL J1458.7+3719@Në<¿£ï^@N°q?Þ<aÀ: –Ϻ¾À<DðÊØ׿È$=Æxä‡@¨ÜRPÚ¹@êvjG¿äé¯z<Ã;¿äiÏ°""¿çñԇðé¿Ûœ–½àåwAGNbll?ïÆ>€hÆ?z$Š‡™¤¥?cœò
/?i5Ù±1\¨?s ññҘl?sáFð
xŽ?ï¹Æ¼Ž
?'8·¿Áð?rh†'±ðq?z Ve3?p´'	P?qÁÚµ&׍?O[ý?ô#ƒ' Ù?ˆÑÿ‹D?'žWÈ},?˜ŸÑ«úÖ?…±ÑuÇj?—õ:Š?š¶ÌZѾ?aÇ/\ÒÑ¢?cqœ4×Í?"¢+|¨Ð?€Q'‹þ"3FGL J1459.4-6053@sÞ
?‰'Ë¿üƌ µ,GÀ6íF4—·AÀ9ûÏÑdB@hzn±@
E\-}@¥€
¿Ý¹›¿änì
Än¿çÿP§Ë¿î¶œxŠðPSRPSR>ûåèqg,¬?ïc§¼n^?ï>
"ÁËb?©í[§"ã?˜7Síª9ü?©D"ym?Ý']V»?2'ºòx?íò¨¯Ë?·\ÏõaÆ?·2Á
ÙêL?·c÷DF?‡AÀn‹?€}2¤Dû?éc\ׂ|?±þ9Rî·?Èÿ"°›ö?±œ
™|m?E[fè-?F?åç5b?ì'ëXYÏ?¬Eœ˜öðd?»Eîoak?¬1áÓM3FGL J1500.6+4750@TGŽÿâ£Ï@L¸®Ú«³À9þÁqN÷µÀ;t7.jv–¿çVjòß}v@ }kœÆ@$ q¿ëŒ$œJ+¦¿ßL©_Fë¿éù"€­ºc¿åø"–ðAGNbll?ïÇÀ܈bX?'áwè½ë?wÒ88l
«?'!DSD.?Q5f
‹%?Zï€:;/Ö?ïµÏþW6d?"='ë}«ú?q•ü&CM:?w/ùÐïU?s'®!?y…ìX‹?îf|¸D¦?"ç‡ÚdVõ?—–‡ø•xq?Ž¯¹ºk¡?›™àþÕÅ ?‰³Tœµ>h?îéêɱŽª?'õÃõG‰F?sáí%=zE?s´ãû??Ê+€~Ì#?"»ä˜é¸3FGL J1500.9+2238@?pc_Jé2@N.µÀ@ÍPÀ8î÷Œ"÷™À;N;õy"A¿åŠ<ïÊ}½@é×µM?þ±J b5ª¿à'Ì!ÅçD¿Øz"ZóÁƒ¿àørOu¿ÕÓËÕzWAGNbll?ïý,Šy?¡?CÒOãq}E? !ö{—"?.€G[÷ÚÆ?-9uŠS÷?:y—'œG?ïÖÌõßoh?vÈ"é: ‰?aN›JÔÂá?gµ»{Cd?gänÕ»Óþ?oñIq)ß?ïg/¢õ?"
›ó'|?}L¤1Ä.?zp³âx?‡æ~˜l	?z 3
FBQ?ïá#†É*f?jBÁšØl?%ÀtNˆ?Möܖ{è?n‹â6ÃÈU?j-®€iÎ3FGL J1503.7+4759@T;[À6ã@LvÊàc'†À9ƀÈè;¾À;›)гâ¿Ø¶á´'@ç÷ˆã@½è@EÀT¿Úªüg´¿å>¶DRÈØ¿ä—$äæÊ¿åŸGïêAGNbll?ïçé¡UZ†?fõêYøÔ}?KÒ7t…?SxàGÞù?a!ÛÈw­?cSãSk®?ïÅ
ØÇ¥?yÇ퉳"U?k"(ª—Ë?pf=F&‰?o_°S²?oÉý^̜"?ïA&'=>f?ƒN2ð"Ë×?Ìøþé?t~Ž0µ°?Ž±_c·g²?{ƒd{–·?ïTmÖðb?‰€·G<£?[úŒàÔ|?W__)•?"²œ`%°-?‰6̬Œs3FGL J1503.7-6426@sɛ€#¦ÎÀ–šÀ
F«À8å¢4rÎÀ;vJßø#?Û毶UUâ@­êY$´j@¦¬ l¿àjÞ|ô|¿ç«
ü÷ü•¿âÄjMÚ1¿éEpÑ4¡®AGNbcu?ï3rO
­'?–´ØɛN?pܨý'Pm?o€TÑfW?•Z‹ßy¡?•N…?Úá
?ëÛ©nlÜÉ?½ÁÚÔn7Ê?'ò®2m?",ñOvÔ?¼~°Ïí?º‰
©$yA?ì´ä4îT4?£ÔufÏë?ŸÞÅkÕC?h$ä"?²a-ri?óÓý<¾?ëä+Êö?£Þýûq?"#4zÿF?x¸ƒ1¬?Â~=îy$6?¢xúw†ë	3FGL J1503.7-1540@u|0¸,,@B?ñ7À9&M±cººÀ;*"ž­Õ'Àý¸à[Ê×@¡nu©z?üPOÞº‹¿àü᫽CÔ¿æóEkˆÓè?©Ÿº"®´<¿Îs0õÒeÏAGNbll?ïÚ÷Ël^Œ?tíݗŠÅ2?1ù½µi?,
¦÷?qd~nƒè?tµÏˆîáD?ïÔ)h‡%Ê?{ý»¢w¯*?_…Õ¢üø©?f"{§º?l¬§[¹^?wC')Ò?îBC–+‹9?™£8û1"™?‰ØAªv?}ÎË)d·B?¥w˜¶áÓ?–p .¿«å?ïå}k?p˜BXe‰†>i|ÝHd¯ú>‡î‹¸÷b½?j'ew·¨¢?p˜7[™©3FGL J1504.4+1029@&Û`C6¶@KJ0 Y;ÛÀ6"bÕ¸-ÙÀ:¨
ހ@ÀY#²·£@"så!Wh@;l0ªÂ·¿àŽ™ë4¿äˆpeSýê¿åRԐæl±¿éDŸ¶š©AGNFSRQ?ï¼xA׍?z¿¼Î•J+?oòÓ1±ˆ?sÜ+ݔš?qÊuìûa%?p(Œð?ïÚÂ&6oý?vïq$Zõ†?`9ѹ}P_?h<^£MÇÀ?e³s?oëˆ×ÄÐ?êŸHDžÛ?°Ì%C‰?µ~±CŽx?¦4ØN  ÷?µÿ—z³?¥Áê1yÀÐ?ïýío®hŽ?FŽ,"9è>ö½µæw=Ø?1ud‰r#?.QN\¨!û?D¼Ç²Îêë3FGL J1504.5-8242@s3Y'ÿÀ4øc ¹HŒÀ:WG6wÀ;·^j¢Ž¿èìãuÃ@Í)éÞV@aÿ ^¯¹¿é³· s[¿åqµ%ªù,¿äÄÖô~E¿å/Ë6õŠ†AGNbcu?ï¦I¸Um\?ŽK çn
ò?cø‰5±'K?jñKgÄJo?oo8HS?‹üÉR!?ïž8fév?ˆ=fí?awî'v¤?l€3²™iI?"ê»Ä»æ?"YҮ̖ý?îJÐ
É®ô?•Žj€/?'bÓÕÖ?-Ùi˜/?¢¡•8z*?ò3ôý<?ï J£
`R?³úwR?B}tíÐb?Bƒ·:êæ¤?›f²¬‡_?ŒîÚdŽq3FGL J1505.0-3432@t¾¬à2Û@4³	¿œb¢À9­&|k‹iÀ;ÞŽ–0Y?ᜏ Ï÷@ ƒ™:@×ýFKê¿èäÜJÚ$*Œ¡—¿ä?[ ˜D
¿ä]cMWKÁAGNbll?ïˆUq^ÊH?'EbÏ»ô?'töþ‹Äc?…P¬ŠßÁ?vëYSƒSD?ˆ³±Såð?ïp`ÊË'Ò?¶Î6@?€nÌÐTÿs?|«_Ow?ƒy|á*?"¹AzL? ?'ÌŠBÎô?'ú&£Õ
?†]t{;Ø?–òÏ%Xê1?†_Õg)Hx?í{+å¦óY?›U?'1LE?•±Î}¼·?ˆ¶e]}x`?­t»>Qì?˜ÅÊ2vf3FGL J1505.1+0326@ä×?Âb¼@I ÷þ½áÀ8…,$K9À;p§I……?Ò	®³@4؉™q@ßú D®†¿å6}âÑ=¿éÿHÂ^¿è иØ$¿æI̧¸ìAGNnlsy1?ï{äa/ê|?'"lª6ŠÙ?€  i?"n¼r®?€æϓñF½?…Ü‹?A]x?í[¬pð½?¸à¨aVÛ÷?®,a˜ ž?µ¿ýŠ¸?˜1¯¦Ëç?L¤Ý'?ì¨} ¥mò?£ðõ;%y? 8\à+?ŽgVÀFÌ>?²ºvÌdzæ? Z½Ò›[x?çw2`±c'?»B¯Ô	¹·?¾eùÿO?³š!¸æJý?À:Ê|?¶?ð|ÕÝU3FGL J1506.1+3728@NÉÍ_™Ã‹@Mò•¿ðExÀ9C×xø9À;É}»Ûä?ò]§rö@"äÀ`Ù@Ÿ+À£Ò¿áõpÙ˧£¿æ.5Lèæß¿è«øP€˜c¿ïü8—Ô¦AGNfsrq?ïÓt"<.A?«Ndoè°?XÚñ}ÎÊ[?YN"$å	?p'u-b?«y\OG?éG5?¥éAË(?™ÂZ˜?¢ žàÂ?&ú#Šc?Œ®$¤¦"?îƒF}¸?–"<<O 4?Ðx«;r5?É5HÙC?'ÆĐô֘?†hÖde'?ì´TñbÆ;?«VºF?´WÒ9Go×?§áä ÎÃá?˜î‰y;?—"KGW3FGL J1506.3+4332@R>Dàá6@M#˜ÀUÆÀ:ŒÅ½äÒ}À;ý¬Y¾O?ËV‰?•}f@
Òæ6«7Ò?ÿ'T€	û?ïð·EçÒ¿Ï"ÑžâH¿Þˆž«Ò+¿â)˜'©AGNbll?ïÜô¦Çþ±?s_`Qú˜?d;hÍvO·?lmw£Ì‹@?]ŸàÕý?cjt†Vï?ïoκÒÃ?'ÿæ$?…LÝ}"J?Šs ÚÅ«ê?}~ç÷"YŽ?€n£^Õ\1?îŅH:%^?TÀÉåU?'½tG"y?‡ösKµ?"'Æ"s¿Ë?M'á,°?î?TüS?¢.û'ûÒ?˜"^çú??"e"žÈ!??ŸŸ˜x{x?›k-jqÇ3FGL J1506.6+0811@!VèË@JiÙÁfgÀ9µ/V/À;€«rßñm?ëNÜ~h@;=‰ù=™?ýûö€¥Vç?ÅUw…úù¿àŸKã`놿Ϯ"ý¾¿àÿ{τ7AGNbll?ïÜÂõ¶0?iÖÉþc¯?d0>#8?b6®"¿?^˘M®?Z
"!áœ?ïGK&p?˜ãwïe?ŒÏ€{ëp?•Ì4LeúX?h¬ºxòÃ?'fá
㣚?î´[Ükœ?'Û¸Gä£à?"Ì{•?‰ºžêgÜ+?•`³v÷t?ƒL"5JW?ì³á¹jbø?¥µ{æ'`?—pÛÿ)~?•ç3=òŸ?´"»T­Þ?¢–÷J+1Í3FGL J1507.4+1725@6ëòÿf}
@L—«ßí;À:—'ï2RcÀ;Ñ<*R¹á?áËÌVÛ.@«¤íµ¥"?ü‰!ACAH¿ïê(¯k?ïšÐsÓê׿Òî0÷wN¿Ób¡éAGNbll?ïüš¢
±[?4}3:c‰Ý?0iC÷j¨?0E7"C?%ƒXòûƒ^?#«Ršc¨?ï´ÿª*†?"þÿÓ_—î?u'Á/»/?€^"µW<Š?oÝaö¶ú?sj–ÑFЭ?ï‡jü¼×?yÜýÐÜuX?{t¶+vô?sž÷û>ÿˆ?€jåÈ´€¥?kºûT>Ÿ?ï'ǽüœÆ?‰99"Ôb?€ì^¬"/5?¤xr(©?uCc¨‹>Ô?€ƒv|!xJ3FGL J1507.6-3710@t®ÿÀ	oë@2-×,uªÀ:	JÅöï¶À;Ÿ{Òuð?Ì1kKÂ:@
«$õØ´¸@jßÇÑ:?ºWZ€Dl¿åH¡y·Ñé¿ÕT…ࡍ¿æ…ÛÊý¥ïAGNbcu?ï#æî®ëà?ž)°ô­?kW(r°üÅ?i§"¯çÝ+?˜=ÌdF?œ¯Œ^ æ?î÷¢›ªH"?›÷\^ðޜ?Š Ìú²¬?…zœí"@Õ?"»œ¤9"?–Uñ´–Æ·?î~ƒé‡OT?"yƒ2Ã?Ÿq«Í8"?€«ÄE¿Z?Ÿ#HÝs?Œò·êé©?ìh¬êï?¡¤ïߜ±?‹'Œ^L(ï?'ü-ؤîÉ?¹Z™åÓl? ¦¿¬Øâ"3FGL J1508.6+2709@D€"ð½@MÈ÷`MÉÀ:YÞ9ÛÀ;³¤ës¸¿ÐŽïnYÇ>@
2ôU¿?ûXt@Éп圏º•¿âj­…+Dõ¿ÅÌò—mx¿Îå}éÃ[AGNbll?ïëAŠz
?iâ*a
6?3"FX(X´?>÷Qr!#Ä?bMìºðâ1?hÜIê]Ž6?ïËD°;h?zeDøѺ?i‡ÐÑV?qK{Ï³ò?k4FôB4?nã‰zG?«?ï*R ˆ?"YZ$¡b?ƒ¬M†Æ?w_Á´}?Ù®û¯h?|	¿Œ?ï‹/n8þ¨?€äŽ«{Q?2Ï¢¢}å?9ë¼.?Œ§\¯aã?€Êؼ'ÞŒ3FGL J1508.7-4956@tF7GMœ@†¿ë½ÔÀ8¥ïm
ÅVÀ:ô"Ýz™ú?ã;Rø¸@C4LbÚ@Ø!¿˜[׿çßsâ3¡¿é÷ž€f˿筕~g1¿èœpc•QAGNbcu?>۞œ?†~•.ó¶Ã?Xo|¡ý?XâÝ9¼K?"IÀǤ˜?…ª¹ý­v?íÅEÕý?²H#™Õ3?`'(qfI?I•Úéù?¯Â‰}'œ?±v\‹wý?ëån¾‰¹?ª'd¸w?ŸJU¨wó"?"@!mnb¦?¹oíµT?¦iwUjz?ê€gïŸ}?ªwèd³Úƒ?Žm›C?";PãŠé?Ä'OÐ8?ª#'±Æu3FGL J1509.4-5850@sÿ?á—_¿ãÄ&½ò·À6ÿ\£oqÀ9ê÷ãÑÌ@äª1xg@¶'ž?ý˕/&´?»Í}þ'¿ß!]
ÞK6¿äÀj4À벿옗A‹Ì¹PSRPSR?5N6*"ý?4Cî+B"ë?íí·Hû?µÌà9M²?°|ù•Ï¥?µÂ2ñX©.?Zv°y–?03ZžùÁf?çÂî«?OJ?ÃFOÓäpì?Ðy/؝«ë?ÃFŸíË,?r']·_µ?k4A\£¢Ô?ê^Ä>ŸrÎ?´ÖÖã[ï?ÅôÕʔyÆ?³Þî¦pæ?mÿK??dŠEV%E?ç) \N?µa½'¿¦Ç?Ñs ÇMå?µaTp‰AÀ3FGL J1509.7+5556@Võ: !Þw@Jߥ¥À9ðE;ss•À;ÉZÆõó7¿¡›÷êH7ñ@¬‹ä¥0§?ýí2?î,™¿Ó»6.\¬ ¿ß&ŸêŸ#O¿ÙÌ4mè2P¿ÏÞÇ}À AGNbll?ïú£ëµ¥?E*Žâ?-©2Հa·?3<šƒB.+?<'¬Í?>ûGúž
?ïÊ3¹Ÿ˜?~û¯Èóš?mÅ†âm–?xz£ ì©ž?ha¿}ù?m¿þ ?ï}10¦~?'"2èû…ã?Ø9ҕ?{÷es@?9®9w?sY!O¬¦?ïó…—-û?tqà^ߛy?3?ö÷Úid?7¦·G[°j?|ò=Äë\)?t5—*c*3FGL J1509.9-2951@tù_™Ã‹@8F߸aÜÀ9›Ý÷vÅÀ;|4*©÷¶?îRJ|ÈIþ@ úô¨^@@âf'†¿é
7a|X¿ëኃ›¿áeEy±Ç¹¿ïýl*±À"AGNbcu?îÚɪÝ[? w®?"!Ê
?"ûl}vè
?»œŠ°?"o
¶Z˜?å6lEæ(?Æ4ñÑΓO?ÑcV×Àœ9?ćVïû¡å?°¿C¾Î]â?¯Ú$†Ùç?ë{¤¦Gw?§ø<|}'_?³œäü®{j? '@ëS;?°…õÓHã?™'¨'ì¯?àÓ4╿®?½YÙ'‰a?Ñ՝8º½u?¾™Ü¢Î7O?Éò3†d?²ÞZ©¹_3FGL J1510.9-0542@vÿÅG@EvÖ@†À8VGõbÀ:õÇþ0òç?íÎû?0å@<k~ÿ@gŽß×@™¿àp‹Ð¦¿æm¡v»P׿æ›\2ÂZ¿è‰.NjâAGNfsrq?çV"œy?ÅoÚa;\u?Äê@­a…Y?¿V{¡]_?»z¶H˜ˆ?¼Å"2Q¾e?è³jö도?ή]g¶?Æõ"×ëì•?Áµ²š
?¨ó=1—Um?ª@My†?èóÁ.Ô?°£œþ"~?µ­À.˜!Õ? BCe-"á?ÄÙPãû{Ã?«ËPÝRó?Õ=àXgÖ_?±ÉMJð0?Ö]
#T¦?ºÜS$¤Îü?Ôe"Cƒˆ?µSÃÚçÎ3FGL J1511.8-0513@v)ä p¸Ð@Epà<ìÀ9F ²'/À;.¥öŸ..¿˜p'Á]O@ãRi.lÐ@EÊ`‹Ûì¿ê½€i¥h¸¿ÜüD£aÞ¿×â†G'K¿á8;ÝÉÕAGNbcu?ïì\¸´Ù¨?nä
ño5?QÙ˞m ?hÑ…Q#¥?UlÂ÷ߓ_?_ 5çSšb?ï"u¬B&3?"6
Q)C?|§?ò'†?{è,ÏËùû?yéìmSÈ?wî†"Kž:?ñF±?'"Z›2?Œ¹'[Ô?'1y"ûÄ?œ¿"û)?â?Œ¨øPà),?í	YÞÉØï?¡oÁ¥û?t督	?o xáMy¸?¶s'˜—^X? ×i  8Ø3FGL J1512.2+0202@¤r¿#N@Gý}æOUÀ8zFgÃ]¸À;@¾61u?æ{S¨)Õ@ÌZÁ¶%@™ã KO	¿á½-'³N¿ã'÷­ßT¿â[eé#¿ã†Õ½à:AGNfsrq?ïÍ¿–ï¸Ö?ú<9gyí?[ðÓí—o?{5ÙiœU?r$4(/1?q6™T*Y?îwŠ†£¬é?¦svgK5? D¤¿b4¨?£ñvj¼g'?…e¬Åùš?ZrÒ²œ?îÀÁ®¨¦?"Ýš+µ
?‡F¡:7ÂW?~=)KÇ?œDy ¯	ë?û*jo?钟s¶Ñ?°01®¢Õ?®ÁSº;kÒ?¡çy:òy§?Â-B–íÄ?­ýæ.XµD3FGL J1512.2-2255@uH^`=Wy@=xœ \–ÚÀ9â¾÷!À;d-–;@H?«†9¸¯õ¬@
®µëÓ?þôÿÆÊ)?ïËuȕ@Ö¿åïÿµ_ü¿Õ"'
»¿Û&ón¢AGNbcu?ï"NÈRÌ?Ž'oXjMo?WV8õq†?U-»3á*Ô?ˆOe/H>›?Žù\Öd?ïAQo?"'÷;¦
%?uùÓÙ×D~?sîÌpY{?2ÁÎøœ6?'Ü"bo?íäDZyçV?›0;ÁÂN%?"\ë(½ô?…S3Áîkâ?§…yòÍ+?–Tôò¬®f?ì;éñ0Ð?«»ÁÇôNÒ?uÊË2Eñû?v—ªÍk»?¼Ä
mRe?«yn簆Ò3FGL J1512.3+8005@\ýÃ?…Q
@A†ªšêÒÀ:›Ò‰¥/ÐÀ<*y®AÇK¿'&†ç
@Œj€ý@ˆ@ò`…%ï¿ë¥ìp¿äø,"¿ã'l"	ì¿ã3-ÇcZAGNbcu?ïêÆªé›?sçáKý.?bþg³ë·?rg‰²&jÆ?3ÃѦ?=½¾£åá?ﰆÔsÖa?€îï¡M?qŸÈ=â?rk	±®_"?v|þ' ?wœœé´˜?îáwççý©?˜ÄÇÄÛ3?™VK/=Q‹?˜dœ"‹‹c?"õo§…ò€?tc{~Ü|b?ïÀÀu'íf?y-oCÅÙ?U ®[͘%?RÊÏÓxoñ?zW™ ç
?vý·Òbj+3FGL J1512.8-0906@uôŸ`—Ì@D?ßéàÀ5nV·œ¹àÀ:¬²{ï@_"͊aî@"$åg£R@" ¿M¿âR´ü²©Ç¿æPH	"
@¿æ—/˜¿è4š7½ö4AGNFSRQ?î&TOF7?³q[YNV7?'%]-¢%Ž?ŽáèèSߋ?©c»£4?±þ­/ÛD'?ïÒ»ûÖò?'—õâæ­?b¥"Ùي^?i{ä_¼ï?jžpPƒi?€óÉz."r?çí§œSVˆ?³ÒJyèO/?²
€ïh¶C?£0hþۍ?ÇD!þJÁ?±'ÈqÙ½W?ïû=ßu£"?[{Òx6±>½ÛrH¬ õ>é
2ÿÑ;Ý?Bù"pO$N?[yãF5½3FGL J1513.1-1014@uåóà7Ý@CžŠÿ¢âîÀ91#ã4À:¨Â<Pg¿Ý¤}6Ñ<7@.ëBƒ³(@ƒ@;ÚL¿çÄëçf£o¿ê‡a(¿åõ—1´6¿ïý°<÷'AGNfsrq?ã4·D1êñ?Ï)wŽÐé?¢ ñ¾°8(?£›_|%j?×Rs?Æ#?ÏzæÎ3M?ï$ó/Fòñ?—±ß¤s?Œìе@
?Œ,…#7:²?‰Öcy?þ?»÷IC3?ßêùW1?´Ç;är
ã?À؛Ó7ÝR?§·JD?ר¸¿2'??´®Y¾§>Ø?àՍ7Ö?á·¨Þ‹?¢:?Ãj?M=4ÙK¨?܄Ûí#?ÃÏë	! ½3FGL J1513.4-2549@u-ÿ¼ä!@:÷_f—åÀ9®P(6ïÀ;¦¨ñü1>?ùX,)(ÃC@GõM?ôò¬O©¶r?ÎÕÐxö-¿ÞB1õÁÛ¿éÝk±åüÛ¿éVcCÇ*!PSRpsr?¼ŸíëW/?¹Îæa‡ô?ç0äS«í?ɽ5³Àéh?Äìw»Ê¶?ÅNi,	‹?ÚhœÃ?Ï…–ÑÁ?àjéþ¤á?͸¾Ñô6‰?´l¦hld¸?µº|~fȯ?Ó=™<gŠÁ?µÈŸø+ÍY?ác'"­™Í?º<‰Ã'5Ô?ÃöÄüzƒJ?­Öٓ·?ÐY4³`?½´io)?ä1«>‡?ÃP6<ܶ
?½ª3CM?´Üo™le&3FGL J1513.5-3233@têµ_þmY@5këß·‹À8úaPÀ;[ƒäün{?ò¬»y"@ÃæÄŗN@¹áÀ¤ËQ¿ßn [·ƒ1¿æ:À&4Œ¿æ×G<Tš¿èœÉ@j:AGNfsrq?ïíu¼Ë?[˜DqŠÓ?UÀêþòúd?Qtƒ¨?N§7ŠíùÞ?R4ÁT–?ïË~s:ä–?{c)ìØùŠ?cte‰
ói?f¬Ìn"N?p†"žº"?uI›+_i?î¹ob7\?''ç9"ó?'g7y'þ	?‡&ÍÞIח?–jèz6v?ˆßFì'?M?ï°ª…RÑ}?ƒ'û""?K_иi?R|ââ!©?'%®@.?'d3³ns3FGL J1514.1+2940@GÒtw@MQ™?׆dÀ:/àÇU"‡À;­ä9ÐÜ&¿Ý"žfC<&@w€*@Þ§ªÿ¿éªASv8…¿ìLû^ÿغ±Úá–¿æ3ɖ¿þAGNfsrq?ïöçÑñ?†/Lœñc?ð²·:Ñ?j—˜èÓ?RçªÆfN?†/j‡©?ïǚÜ9µÒ?~óÉ×´Üb?jÜhm/žú?t¦
Bmì?mˆ»Y[?qIheß8?ïR úÏ=?†˜9çìàý?uÕ<[¼¢?t<ËCôµc?yö')B?ƒznXà?ï'štѲ?'§»ñ²?=e¿§bÚË?@Ãþ_X?ŠÍ«e|Q?'bK¬KNY3FGL J1514.2-4947@tS°€0<@6™_·ö|À7ßÇËÜÀ:à)q'@å[½•ø@±aˆŸ?üûòª,¿ÓÛ'~Z¿×Š
oª1í¿á"Á0¿îö¿ëhdj/@,PSRPSR?cµF•ú2?b$J(Ú(–?î´#‰õT?§šHèøo"?£'v>«?§߇ÄÓâ?HŠŸw?`æMèŒê?íL•VÆ"?·£r¹ÀR?µk ;ÊI¬?·•:Ÿ"<<?¥gÀøT¶W?›†îr…–?ꉻ
·7?±¡'þ¯U'?ÀìÕ³õ‹?¬
‡yÄ4*?q3逿?kg"Fh?î
ñ>?Áa–^Û/?­9#¾÷Ô<?›Úˎ|Ò3FGL J1514.5-4750@tdñà'Œ7@ Þ#ê¬À8ÅÅ.î*À;-R,¾?ãË4ôJât@àjR¯$p@£q ?[¿åݕH•ßÀ¿ä­8Íw¿àõ6â%Šº¿ëF'9LAGNfsrq?ï'>Š<Ê?…µõ+¿?sg¤….d¶?q
+;ÈA¶?ü‹<™›H?¼&ûÏ?ì
ÓñÌÊ?ºBâù,‹?'(ü_<ó"?Ž~…°ÐÌ?ºÅRH¢\â?¸ï[)ZÝK?ìž=ÑR)Æ?¤–Ó
?©šg'`@H?™‡Þô2Ù?¬»h}#E?™8%£pÜ?ì&¦ðÈ?¤=·éó6?ìÜ&aJý?†Ñ°ŠZ?º˜=È&ø?£'Ñ­žr3FGL J1514.8+4446@R‹UŸÚ%{@L7W`9%»À9J\OÝÀ;ÊÅ-œ}?íúgPàÜé@ÐîÕÒ°@¶G_eY¿àa·ã[¯~¿å"ÐèBþ¿å™‡¿Á¿ëU'Ö¢}]AGNfsrq?îäԛ&?œF
©†I?›h¤c]_?™EŒµ·Äå?€*Á¾o¿g?|3_m;¿?ëê__g­Ò?·
ªØ»‹À?·ÓvÄ3"9?´'1fMP?¡³úx?ŸtE,é ?타!ö¡w?¢D{Æ6!?¨ØÙÞ>'é?œ3øhW?ÞH®«:?‹ê߂³R?çþ÷®ëÆe?²v=2‹ˆ?Èœ	ž–?¬uÎÊæõ?°
VŽ¬?¨™¦üb×3FGL J1514.8-3623@tÊ # –@2Ù_'F—À9ë>nИ3À;‹<R–¥É?ê©idð@oèך[6@=¸¸ÇÝ?âºT£‹¿ç,.õ¿gè¿ælõùÕ¿í/_[&¹ AGNbcu?æòZ6Bp?È))󊒇?ÎâªÇ(ñ?ű›"?±«Ÿü
B?´™€¹£Ñý?è0¢Ô\†?ÆÇBXçÃ?Ž#Õ0?¹QÃZÉu?¹^­óo?¾ëház¾e?甂ßÏÐ?´W+¹^y?ÄH Ì2KZ?­¢ò«×¥ü?ºÊ©èœêÊ?§¥ËÚ¸}6?à,
A]6?¸Ä=Ž*«ä?Óÿc=dY0?¸@.Aâ™Ã?ÇQÂuX?¶¼Î¡'³ƒ3FGL J1516.7+3648@M×­€k`@Lô¯ÀL‹ÊÀ:s[Ÿc6À<
ÅÓ´G›?ã'ã鸯£@Ö;‹qc@שjÄD¿Ø‰Ö«Ñ]3¿â­vû¿åuÒùüI¬¿ïþ;g4A¦AGNbll?Û¸7?›uª!/A¯?Œ½ÈžzEÙ?š­GBByÕ?RÚä½cD?jiæ¹^²ä?î†.Òwó?¤ñY=? /WlqƋ?¢6¾ºsÞ?¶íɚèü?‹´F<·ò?ì-=IØ³?¤òƒÝšÒË?´æô°«?¢6ñ¢s?£^CTSÓz?"&BDbé?í7ßõN_?¨;PÈ£f??°'<ڕ²À?¤ù1ˋø«?–»
ëÝS?'ª^•.+3FGL J1516.9+1926@;՘Ÿž–Y@KëÀ·pDÀ9Öï
wÀ;µ"'±ÈÀ¶:¯³â@ül¦œau@#ìÀ24±¿ænž¯¿1¿êæíZ¿çû÷–5GF¿ÜÛý`':œAGNbll?ïïÊÁ
ß?cÂôžýr?IWF‡Ûl?JÒÕk€Œ0?S¾Ú€^Tä?`»b·ß[ç?ïÏÇðü?|KµÏ{'õ?g"¬Å$¾?sè÷ä¨Õç?iùb>Óé?ogE¥§&w?îæÁ5fu?‹@)Ñõ1?"w1LÕÔ?v$ö·&D¤?˜ì@¬Ô
?†%wtÝ6?ïÍ´¼‰\?wAKßï
ª?kåX9?ÊÈ<Z‡[?xïƒIñ:‡?w4Œ6sö3FGL J1517.6+6524@YÛa»û@F³'Àa"À9OŽuy)À;L	ÃÎ!¿õ`‡·™ß»@sIcKSæ?üƒ—
&Y?{­5F¢•…¿ã-dÃ2¿Óƒª3ða¿Â~	ZÇ¡ÀAGNbll?ïù-ìï°ì?E?ŠG.I?&Ý󧚵?$2÷ÄÒ?EÏÒeÆ?CQ6œït?ïԛEOµ°?w6 g, ù?eX]ˆ?l"»ë~T?fNŸ§ñóò?m|þÏ~Ð@?ï>8øùÔ?†ØþšiÑP?ƒ‡ÜÄHø?}Fæ0gt?VpäýB7?fâ…¶?ïÌ ™Þ?rßEçCˆ'>ì¾ö'QRÏ>öY…xÙx?y¡'ñçí?rÛ4;cét3FGL J1517.6-2422@uJÑ"Dž@;"§@KIªÀ7es!_ÌÀ:ÔÖ-žž¼?Õû¶_"$m@eÓ|"P/@å±_³ï±¿ã#oڔœÁ¿á¨ãîžÑ¿à
¯€ƒ"¿æ"YO@tAGNbll?îäp{K?¨ªn\"ì?‡1Wâ_5?ƒ£aD´"?©xbVSŠ?§]îœ:T?ê§M4½ß?ĉž­s?¾ËCÞÌg?¾Éýq(ž?§ô¥¾–‰8?³`rÞ#¡‰?ê[Ï;·¿?®g­y½?c?¡jm¾«ƒ?"I‰K¦~?Â6Bµ±Y?©´Ri2`ö?ájÿjfªñ?¿ö…ƒP?µ½(¹@$Ç?±¼jL
áÕ?׺¶üâ ì?»¬rGük3FGL J1518.0-2732@u*­ ‹]@8ùx¿.~™À8šRÙÀ;$C£Ã¿¿À€+q'Æ@"ÂLÁ#Ì@‹Ÿ°ßÜ¿ÞcS÷ÎÙ¿äâ=X¿Î{¿àÃQ,(¹¿â>*þ0rAGNbcu?ïøG¼+ì]?M>?%ýç.?–t=F
'?ÃwXÆx?K®@È¥Ä?Lˆ<Vžaq?ïÄHþp1;?~¤JȎˆ?hˆ'¤+ª?jÄ«¡…?q—?ºM¹?vüÏ%i#œ?ï?ã	m;?ˆä"¨pj(?y±¡Å€?o¸»£"¯ˆ?'—6aXn?…rªƲº?îЃYlÂ?'ÑC¢T¿í?MäêÆL%ý?N—ådøÒÉ?¢€6¾%#D?'®Š%Í3FGL J1520.3+4209@QG¿@OÂ@L_×ÖìÀ9³—>u‡À;ÝWªå?ì/xB~L.@5¬µ*D@ýXÌ¿àv›"_aÔ¿è¿\"ÞýZ¿çCvý<½¿ìPa¼Þm3AGNfsrq?ïðø´ÈÎÙ?ZÀF‹»vX?T©Ä°w—"?V"ÜBßW?BÉ£{Õn§?C@4m:Æ?ïPhÁP¸?'+Ý߬> ?‰»8ýû?Š=…!D£B?'*´"ÁSß?ãuîíMŠ?'¬?"|,$í¨?—¤þ«,x?ãi
8˜ð?"ÄϨ¿P}?†`,;/€¼?íùe™¹:? þk¨‰ûø?¢qz7ǃý?"¸¶;öd?›ðXpи?™tV]d¹ž3FGL J1520.8-0348@vaä?åÉ@E@Ì?ß À8ñzbœ­JÀ;B…¶Æ?ìù×	Å.P@þC"¨"Ý?ýXà¨Ì½?æ6Ãì±ø¿Ø¼c,9ͿΕE=-­¿à$¡Vk5rAGNbll?ï§ÆM?G±f5?z1}.}:_?y¿zþ—¶Á?rDÎL?‰^YÌ8L?î〄Ì
?œ¥VŽ¢·ô?—)éۗ­?•³S7Ná6?ˆÌΚé?‹Ÿjà?í$'"£Ú?¡àÆdO?¡çf{èJy?'r òYþ3?«ÏpIæWò?™»Åv©?ç{ìq¤?¶ÄŸ~tê?¬-µ÷2íj?¥Ä¶2©6‡?Ë໣?µÔ)Ê­3FGL J1521.1+5543@V‰?ßéà@Id›`C6¶À:{7ýJCÀ<#ǃ·°?á&D"He¹@
È—ý¸'@]+éTm¿ìQßÅC'¿Ö.î"Fe¿å=äð¥¿Ô?Áœ"[AGNbll?ïTä~?£j·W?mÀ?'êætúb	?£ÕmG—œ?d'µEHq½?c¯#Ö8 â?ïP0•ðÁ? "õ'fd§?‹Ä©ÕðÝí?›ÁH܈ö?€/0­ÞÞ3?ƒ'Äî÷à»?îƒQ_Óö	?˜G<ò5I?˜²úÑ»'\?"rÂ;òI?–âÙ3ż±?"B \ҟ?ïÇg'?˜&׌Ïä?Ò‰Dø>?'èW®yÔ/?Ž»œ+^?ˆùœ'Á‡3FGL J1521.8+4340@QæïÝëÙ@KÉN ƒyÀ:$ìH"ÉÀ;×#{/K?×ÜŒ{›@u^>#Ò@Ú÷àvͽ¿æß+‹7ðÌ¿ëš{Òðd¿ç^õ }ùֿڕTV0ŸAGNfsrq?ïã[0²GÎ?¬GI\??Z·š"¢Œ1?š £Õ$³?^'xÍÖÈ?î	œç?ïÁ.'K¢?}¯ŸÏfFQ?p®FÐ[?uWîi)™Ë?m·ì&¿'?p§]á°Z?ï{E	Ãs?õÒ¬'=?vô±|Åw-?sg«S÷L?…´f¿,gÊ?xñï˜
?ï¤ñ'û?'ƒÍÄ
@i?Xj™åÅ?]¼¡Üúõ4?ƒúbŽeD[?Wd¾¡
3FGL J1521.9-5736@t VàL'¿Ûd _þº¨À7d˜$ qÀ:D˜n#Ê@d—.Z[@Xç×Nl@=Ã/@¿Ï•¦'Gã¿áǼ¸é§4¿è}M÷7b ¿í ÞW
ØÜPSRPSR?+aH¿)¹M?(¾ËmK·??îžÚŸ}5š?®øóQ&?¥öô¿m|­?®î¤ÜGÐá?
‰á†‡'Z?0çl6Ã?èÿAZæ?¼sph9z^?Ëÿæ\}_ô?¼tA2ü.k?zŸê	UC'?o"=A³Äç?ꅌ=¼‰Þ?³tï†AÂì?ÅϸÃ.m?³"g×­"?n¼¯Bá,?cæÎր"y?ë<˜è`Ó?¥'¸'Ò"I?'©¡w.?¤À9FØ	i3FGL J1522.1+3144@IÓßæ…@L'ßý`éÀ6FchÀ:£ÓöeM?û¨w³?Ýæ@…éµí¸@~ÓnQ—L¿âN¬Œv¬–¿åʍ¿	¯p¿æ]J "'¿èÏÅÇíAGNfsrq?ïëâ?^'/ù¤?Z[Sùéü?X¨ÄíG?KŠáÞ>?IÃTºï³¼?ïØH÷îrç?wÌË:¯×?ac*DÛû?i{Özw´?fSÞH<Æ?n–gZ7÷?îv´ºöé¦?1ƒkXó,?'[~…K`?ºÛ‹õm?žÍꞝÝ?"ñŽº^a
?ïÝúM»Ì@?+¤›6?4cä~?PûÃCyÜ?o…¥à70?~šÊÆ}è3FGL J1522.6-2730@u9\_|gZ@8f6îÍ©À8$l"}ÐæÀ;žîm0…?ò³üY,l@Öâ'ܼ@"à)ËÖ¿Ùkë[-M@¿ã^¢;˜vH¿àTË«±ì¿æ´œ.ÊBÚAGNbll?ïñú@ì?VZ'Wùö±?:""õ]ýç??.uG¹i?U'÷t¥]?RY`G#õ?ï»åß²?å	Oà?m^œ?nŒfƒ8?sƄì$h?vŸÔ¶U?‰¡ò?–‡nu§X%?£ß¼à+?ˆþ3XÚJ?™ëá'm?|œRSx?î…M‹_»p?žË"ë?rø%³àsF?wý OF¾<?¥L""ˆ:Ž?» U3FGL J1525.2-5905@t8–ž=¿þm)Tc¯À8äç
À²ãÀ:QÎ2þZ?Õ®ËÄu@
½U5'@JÛ`cm
¿æHP¯×ï¿æ©³ÍÍRÚ¿ç
'¿ç-BÀÜ1AGNbcu?¾@ƒ; F«?¼ª‹ÒÀæ?¹•¤üq-¥?¼)˜}á…Ð?é:øýÑv?Æ
¾»Äޙ?Ô¦t?Ò`$ä N?¼;	ËÄjì?Á¿­Ê_"?ânË¿Mcš?Ò=¢I?˙þ4Æ¿?°A/_th?Ș! F½8?±M5÷•t?âó—¸a?¶äêá¡É?Û³"9'?Ä¡ô«´?ÔڐŒ?…vŠ#9T?á¦æ>xöx?Ä|aÉEZ3FGL J1531.0+5737@VæPß´0@HS?Ýe¡À:y¿ß~€À<¥šXÜ:?âÛ$»#ù@q|ï>çœ@%±ÀVò«¿çíÐ
¿áœF7¥f_¿åRkuwƒù¿µÀ½mÍAGNbll?ﻁßxÉÐ?'3·ˆ.;?~š%i•º?'`ŒnÆ-?PùØxƨ?dՉ=¸¥?ï·[»CÎÜ?'1Á¿—ç?t×EIwÓ?z˜šy¨t¤?p;KÏô?qú9c9Ô,?ïF<ü#?!κZ,y?óp~du?‰–AM¾é?‰m}‹Â'¶?zöyIä?ï¨hËgl?†N?Ln:?b©…Q¬<£?m–³!ˆÆ?;kѹÑ?ƒÌßrRä3FGL J1531.8+4704@SýÀ?`@Jr¢ŸÒ˜¿À: NRsj[À<ò¢Ik"?¡øsìý=@
ð*IÏ,@†Aßsm‹¿ëÜõB¦‡ƒ¿Üò4@à¿æI§­Û¿Ø
«(t‹AGNbll?îåPp×ù?´Õ¤7å$? m А?³ë,ÑÉ*?cՆ:þŽ?dÒû1̌4?ï¢\›³t?Š¤Íƒ#´?yµ•zݐ?'fЀџ?u@<8"h=?xº ïÑm?î#¹swä³?ž\ÛS–?Ÿ¦0¼M?˜U‡Ûý&?›â Ô¶[z?Š9S˜Útë?ïŽL·ìT?ƒpDQNþ?qlôJ¢?r6ˆ¾í¶?ƒæÂ
ÅÔ?6"'.õ3FGL J1532.0+3018@Gì:?–îÄ@KhZ&–mÀ:!=ÍÀè"À;´:ƕ?Õe™W)‡Ž@[¦nê?ü>AFœG?ï÷aÐu‡¿Üh‡Š…¿ÑY¤£°@G¿× ‹ŸÊ¤îAGNbll?ïóÛ¹¾¤?XÙ·Ô>Ëê?G«n±š8C?P>ç]Â?HåªUû<¾?Iœ-"M9?ï«%žZä|?ž«¥?.Ï?y5¾îô>4?Ž`¤Äý±}?q7q㙃F?s,¨S&?݇?ˆ åó]r?‹zpáa¨?':MPÝ?ÅŸg<?z´[ª­c?î¤ÄïÓ?õùWz²?uˆ¯Œ@ÜL?y~º«¶˜;?£
8'(ç@?œ4¾Íeö3FGL J1532.7-1319@vHÿ¸²d@@Ü
`:Ó;À7Ý[+J1À:êè'œ&<?èݯr–Aî@@‹Emó@À…Ü.?¿×!R¦ý¦¿á"­Þ8ô­¿ãÄUã4¿ßó¶ËهÆAGNbcu?ïúKˆÑ°á?AŒ«`ÃI?,ŽyFãÁ?)IvÍ@1??\|ÏT?<B÷vâ?ïÔ¾Žò¶?y‹Â@?_Â;lÑ&B?eDÅçc{ø?k`SW‡¶‰?tbàQL°Û?îhBÜ%Ç?–wÁ
¾³?ˆê&ªee?‡VG6u? ÎòOS
=?'½¸{ñ<[?ïþfŠ¬úò?7Ïìƒ>—'@"¼u>´ª{T)%?)‹Œ™Þ?7͖ 3FGL J1533.2+1852@=)@ªÀ3@Jÿ—$tÀ:0;eÀ;¹ãÕ'b¿ãùB¦Ì;@
ŏb^?þOà2ZE¿é†lêJ¿åÞŸ¦Eq?½‰Jl	éc¿Ûù˜áýzXAGNbll?ïïÚóT'?`]Š‰£°(?& Ñå8³?$›nlýám?]v=•
M?_°h@C"D?ïÃwÔd­p?}í툍l?lú$ókÚ½?r}°·5˜?oŽ§æ´?t;°nî?ïNÉwŸî?€y^û¥
ý?|[Îç>Ò÷?o3<äl]?ŽºÆx›?y½jÛlj¡?[ß ?€Ãˆ
¤ü?>èþJö)?&³$À¸š?‡(k6='?€¸÷åP™3FGL J1533.5+3416@K_{Ÿ³@KU@ÿ¤nÀ:lÃÕ­FÀ;ÕòJ4×x¿Òɐjc@¸©Ý3¢D?ý«:ÞÎ,¿ãSÛýÊÏ$¿ç$8vi¿°T÷†½R¿ànG˓RAGNbll?ïí¤ÂËm?a4ß®æÜ ?,kø"ª?+cËÎ3!?a=ä}²r¨?`·±tAö?ï²Q¥ æö?'×/ábš¶?t½3?Å2Z?zÜû則?rùïÇRb?sc{O¼å³?ï&7áX[?"aU…µµ?÷#†+Xý?p§ëßZP?";:órÞ8?~󥶉é?ï["ŸžÅ?‡;'¼ï™é?C­í>çWg?L…ÚÄF?"LBì¥?†ë—cDz3FGL J1534.4+5323@U`7ßÕ¾
@IE`\a*À:׺nü7À<!x#'L¿Ý•VpqyŒ@uuœ9\?ÿZÞ°t|¿í9"ZÌf¿­š"i´¿ÐIÀ	è-ž¿ãŽ…ÎØâýAGNbll?ïé0ŽÔS|?{-ÜlÈ0?b–'K'Ñ?xžñÁwÛú?@å''Æ?P#x1yÑ?ïƒ@RJ[®?º7!?'‰à…;'?‹fF†¡Ö?y\ÃDz?{ך
)í?ï)H©¾Ë?'	å…q1?àÂUØ?%ëc}?Š4)©_¡§?t¡–q96Û?ï£ÙuÛã?€NM?üÌ%?cJÛøv¿?b"'Rö?'6ëŠé‹ê?|Ýß^–+3FGL J1534.5+0128@´‡ßÝË£@E¢¿ÖDEÀ9r´€ÈÀ;9oV•¿÷RH¿·e‡@ä8¤6V@:Ä@]׿çõ*åd{Þ¿ê%…sÌοã2¶¨ö¿ïÿÂáo#ØAGNfsrq?ïþÔGÐÂÕ? ¡J4Â&>ÿZ"S>ü?¶DQ<? &åv´?
/ØGê?ïÔT¸·Í?wˆuð®"?bïºJx †?i(å#6?h»ŒþhQ?p͔*Ú°?ï:›˜mù.?†³
GIù°?…¥`sW?yaP8½­?‹³¹q*žJ?€¸¿S¶>?ïҀ*=+Š?~e‡n÷Ïö?"Üx¶‰'?4ô,ˆPN?v)µît?~7Y=ö3FGL J1535.0+3721@N: þ¡@K.ßç[ÄÀ:kc%iFÀ;èa'ÑÖø¿×IñàO@UáŒR3@é¾ RÔ?¦:A^2ÿö¿ä0+Y¨›s¿è¨ærT+?°+n"ï¼AGNbll?ïž9¿,'?"QLßmOý?€à6µÄØb?Ö¤³XQ?nEfÀ?tFý¿ %‡?ï»g®ó+?ƒG'.¼ao?r;0X߉×?yzÏípó?pø¤&áŒ?v[5{yè?î¥% ë?›ÚÂSË ­?¡B&
oÃ@?–7CdByÏ?›çB¼\$?‡÷qIÀçÝ?ï˜*iß?‹Úɒh?Rg[ E?_uÝå `,?‡¨zW"16?Š=Œ¶²"3FGL J1535.7+3920@O«"?½…1@Jó®ñðÀ:§ouÙ ñÀ<bfýe?Ý©¥wÀ£@@d•Xí,@Ë.@/E?ïþ¼I$"½¿Ý³"ê÷Á¿ç>Ԁd-@¿ßÓÜW>ÅAGNbll?ïiBŸºhó?°£à¶¤€?Èn
¾à?°mqü}Ÿ?eßÕA%?€%•Uؤx?ï€m ;?"q'zÞÆ?'WË¥‰t¢?KT¦·F?{Gæ~ùB?€/›ɚ?î‡é³3?É‰^þmÙ?¡h'˜^")?—_eU¦5–?š>³˜Üw?‰¿Hš~?í¡¤}1$n?«Åˆñ >?¤[j¬Yø¶?¡QgŠlD?¡ŠM€"ÀT?£5U±ÙÙ3FGL J1536.3-4949@tƒ!_Ìr@ Þý';À7)&p­À:"&êþ@&»¶Où@y6R!Šê?ù×2
ï+ò¿Ù+¹öËпÜh‡#±q8¿àKª7m÷Í¿é=ORòPSRpsr?žpû›èbÎ?œÖ­Ýc?Ó7Ýì`?Ìé¼ØÕ?åp‰—*Œé?̔Ä#S?ih-H*J•?{ÇJ\uÉ?ç@G6É"?ʞîÈ;E?ÑL¡7ݪE?Ê}õ ]!¦?ǐV}ø"?°éɽµTö?ÑÇ3/I6e?µ+g°Iå?á8PÈÝAi?º	è8£Ò´?"enê`œÍ?‰ÐT"áýÉ?ç%EÞ#)?·nwîÒ²f?ÐUS¯ß?¶Y
*ƒœk3FGL J1536.6+8331@]z÷@?åğס<À:~†TBwÀ;ýF†Í;¿ì°ç¶Tˆ@ìF±c@ÙH@`˜F¿âD÷\݇¿çð›nª¿æboð9Á¿àâf¾O%AGNbcu?ï²ëuó‡?™"	z¡êþ?p¤£\$m?™IV/.†?uå¢}ª6?sªë´µ§?ïƒi'lK¹?•&ãÔ¼_?µ&vÚs%?(ƒx1y?~–EÒÿ¯¶?"eö‡©?î›)•ý?•qóŒ"?'þ´¢W?'rý˜
Z?¥+ü:Ø»?!e
jåß?ï4Z"*?Œß²˜ÖÀ?^}Iº½s?\%‹8´?—Œç!±1­?ŠÐg
V–j3FGL J1537.8-8000@s_<`ŸÀ3}_²?À9CÖNUÎiÀ;~æ"ôï+?Ö!ª°ÔYð@KÚsÿV@}Ç/$Ü¿á¹SK~ó¿ãgâ(Ý"¿àRÁՑ±2¿çœì='AGNbcu?ïÈXDþ@x?t¸[ò"?E'ÞɌw?D½6¼ähV?y.᧮5î?s§ªÝùK?ïfë6E²?"l"‰··?oðzö]-?q³B>»2?ŽI½WQ‹?'FøRÚIæ?îÖ܉'x?êqd?†i ©ÄÉy?x1)p{*
?™ïžŠËLA?‡V®L?î=‹ֆ'?"¸–~{6?n jó
¯?d™@¾YŒ?ªEGèlà?"6ü^ÝÆ3FGL J1539.5+2746@Eôv?ø="@Jqÿ΁ÙÀ9O~Rì6À;šÌÜ­?é(·²ù@Ésô–$@©:ÿZh¬¿Ílï)÷}Ù¿à¡_ðÚÕ¿à›Ôÿ˜ž¿æmá|S°AGNfsrq?ïûÒ`óè?5ÝoÓg?1]/õÉÀ?+¶ØP˜?0[0Éþq?+S,b¯c	?ïÔH\#F?wª,صH.?e]ÔÙþ?lLª®Ü·?f¡FÊßß?lòÁoC±¤?ï-Í"Ÿ?†ð®ÀØ"?‡'¨º c?•´€$º?	#åzµ'?|¡½G®0Õ?ïåTÐ*ƒ?n¦€[ù(?1åV^'œ?<Fô/9µ?hoQd˜*?m´½Ï¹n3FGL J1539.8-1128@v2ï€Uûµ@@çk b
·À9ò¬U^fÀ;s×gZ'¿µc9ìLÿ>@
°R°Ñïv@­Ó %¤Õ¿êȆ)þ¿äj©…䠿ݨ"õèF¿äé£Rˆ–›AGNbcu?ï+Ė?šóàAVìØ?p[ÛÌÈ?nS"`=I?–pvL«¸:?™"®°?ïmw+t>Þ?Ž+kÕ7?'Q%
ü»?†ÐçöÉ?'QâK»?'ÛIu–:ý?îv˜ïÒx?"VË¥ÿ?ŒÅmó°?{òYdñi½?¡e†·,?¥Ñ"ŠÍ\?íRß!÷%?¡±›1Þ?|ߕ
ÁTð?xh‡.èô?µ§o¶D1€? ÌKu'±¡3FGL J1540.1+8155@]—¿¤Æ@@{¢ò(§À9‹QÿÅHÀ;}êXÎÎ?êú"9!@T6
-?ù¢ºÀèG?ïøœÀ¯K÷?£B†jñC,¿ÛèQHÙ¿°wËNٓAGNbll?ïáÍSÀ?lΉ@Û?fio?fOM™èÐ?QÚDzI"?[ÞLK¬œ[?ï°çXBê?†pÔSi?sIµ†?zXôpÚÖ?t†
ö)¿?<pîä^n?îdiÙ\1?•Ž*+ù‹?™½€¨+F?åkd'Lx?™µD7©3Ð?‹^Ãvy9?î@^ø¥‹ü?£Í9ˆ=«?Š:¯iì¹P?ŽNíö×!}?¥kd›,Û?¢ýêÅ¿©3FGL J1540.8+1449@8`Ÿþ7©@Hhâ:¸cÀ:œU5¼À;xÔu§L¿°Çñm<°@DYgzb@ÂgŸÌc›¿áè+ðɬ1¿çPÐò@T¿éØi€¶}¿ª­eÌô¡AGNbll?ïqéو×?"Ð?Ùa¢?t·à^™¶Ç?ƒ_»kCY?‰)™n}_Ê?Y5ºûP?﹅¸G˜9?‡Z5[Ó'¬?s,²2'Ö?Ìx+‡3Ä?pq©¢
Ä?tXG0þ^?îJ¦Íw?—[•£—F?•QK˨;_?‹*`ßã¬Î?£¢¯¹¯
Ð?Ž›ßqr-?ïa¹•<?'î.®ošs?Y¸I¤RY?ez¹¡¨ì?š˜D3G?'ž+ï.Â3FGL J1541.8+1105@3Š"€,á
@Gw±ÿÁìŸÀ9ÊÂñ·üÀ;§À)P[b¿È`®Å›@P‹RY@Þ1àwÏo¿ç>O"ùÝã¿ç
dHI…¿êÛí›=L€¿ïþÉ|w±AGNfsrq?ïɤ÷é÷ç?­ã±©{|?Vº¹ê	Lý?UĦ°˜;?u~Ր¹d?­è肢Xœ?ïhV2Ƚ?ŸŠñ»4v?"'vÍÈ?™ŧ€vö?‡ÂÌF`5+?‰Ö˛ó1?îÂoŠ#?BÇ"òî?"uˆ""ÒÝ?¶\ôP?"<–ú*(?…ãϽ·?ìÆÿ"¬•…?¨ÅL¨+¾?§°Ӛ0u?£96mÿÍ?«àáœw'? P½ï&Ÿ@3FGL J1542.9+6129@WØØÀ  @F²`œ˜RÀ7Óû-2h2À:ì³Z§?óòÈê•	½@~b«0E?ýKê"_¿Üؼ'@¿@¿ßû)ñëë¿ßJ:-DÔ¿â½'{Æ}†AGNbll?ïø‹Û쇐?J£›¢cj#?,Šì£?0†ä§Òÿ"?F­Õ%1?E™îD?ïÒ™E	 ?zâíZƒ?f<︣Åe?p¿I»™m^?g¶wS?n—ìÏuw?îÇÈÉ­ß?•¶Ô!Gß?Žñdù½™?‰'˜Ÿ¤w?—Že—âEJ?ŽÑÀ•°6½?ï©éaø‹ò?"rBȍ?A$Ùs'×?X-sß݄?"sYñ…Ñ?ƒï)LØm±3FGL J1542.9-5141@t~œ…×E@Hm`€žKÀ8Œ7ùk'IÀ:­AÞËÓ?êaV8¾.ò@
h•»=®6@èMß[ð—¿átŠô¿èÝ(œx¾z¿äˆJYj{¿íÒç‹BûPSRPSR?¥(‡Ð¦›?©p¹PÙ?´IÇ¢¸Cþ?¸–ŸÇšœ?ì$>Žž•¦?¾ƒA+4$§?ºk*ê¢f?À£J½ªà?Ñqw4mK?Æ›.¼é9?ä×l?ÊÏÕZë1§?ÊÇ,¢"?²uÃО?ŧþ`AñÈ?«¬…Þí?ãä5?g»?¹,,Ð(#?À²Q‹'È?§ãû€?è?Ï·þA÷¬b?±ÑR,!ât?ãål¡´6?¶‰&ù
3FGL J1543.5+0451@(|ȵ1¦@E²NŸ CØÀ:,ÅÜÃkÀ; 	Å{Ÿ´¿õºD²6žx@
¸TûÛ?ÿÁàþ¿ëL "ö¿Û±WšŠt'¿âTÃRß̿ĸÞAGNbcu?ïôĹ­ÑE?T¸N²Í¤˜?>"('ò<?=x¦:»M?M«Aâ…?P<zãºÿ?ïÐûœZüÌ?w¸iöN¿?dãìy¿Òô?m`÷gþö~?j w+Ca?mÒ9ZWûŽ?ï-SWÁ%?" âUKH?'§±†a1û?sãhø¶?'¼DÂt?|ôb5q*?ïÇIéè/?uEý)0í
?`T02?sDãYpï?|0JcˆM?u@h¤(Ö3FGL J1544.0+4938@S̸`.>@IŒÕ£5À:Zäd™ÍÀ<åB¿Ã}}!éµ@'‰¹QÅÅ@j¨_°ٿ׻ϣZ§Z¿àe-Qzy¡¿ëòÀb—`¿Ã‡­,@ŠPSRPSR?ïäNèÆ«è?kŸï/¸K"?]^Q*n?_ìGæ~?ZÝH"¿Ö?cQ—<œi?ïàÅÚ`ö?s¨–$DZ?PlÿuÒ&?Wnýñˆô?gxjµø?pÌEqЀ*?î®ÌžšºÐ?')ã%Ö5?p¤%é?ƒÙypÕ?›n汐?Š'Bîݼ-?ï-?»ˆ†?‡õû/Š?RÀOõi…?]Q#GÂÀH?†\¦._1²?‡xú'ú3FGL J1546.0+0818@0ÄßVø4@FWM@$³>À9°åÜhKCÀ;`üÀ°^Ø?äfIyà[@šÁq¹?û
i€L@ ?ïî
ñº[Ë?çJü©š~Ø¿×XŠå:›¡¿Ö<]ÍÕOAAGNbll?ïùNDÉù?L›'ȯó?<òJn*á?CÇYò3ã?8›B#ß$?>>íkÿNÙ?ï•VÀ¼?Žf+ÖfŠ?€F †?J?ˆ ͟<s?uDH^ï"p?{´.»øt?î÷æ•ve? ƒÇErü?‹jïqô½µ?…~fôÕñó?"Mµ˜8ÿ'?ˆFØæB?î
µî©3?©ý˒RhF?¡çö+wW?¢ž<£Àpq?œirP3ë?œî@YwYC3FGL J1546.6+1812@=í2ÿ0Í'@Hg¥€W©4À:Gç.wâÀ;»Ä4wÖÑ¿Õ¼ùßÄ:@
Yžk˜y@gnåhz¿ãÉÿ&
}¿çf¤¢"È'¿ÐoXÞša¿Þ~K¸˜ÀßAGNbll?ï‡=7Üqk?"žEbíH?O?¥>[vT?PØôXÌ0?Œ<·´ýí¤?"Eèé.~¬?﨔‹¦nØ?6·¦F¹?yärù	'?3v1*®n?qÑG3¿3?s"ht[?î~õøé¼	?•u­ô¼t?ÀÃ!Ó?¸yÖù$r? Ï°Qsvó?ùG
otW?ï\¥7DÌ°?…k3¼{?G×|¬4å1?PÏk²ëÝ?"¬2º?"ªkV}ÇW3FGL J1547.1-2801@u|€àe0@4•2Ÿ|àÀ:MÎ_ªÀ;ƒcÎÜq…?ë'éýÎç@
üF£ÓYY?ûRÄá
x¿ïÍ3Ó¨Dh?ïø5£®h¿á&¸ê¨æû¿ÝG:SZgwAGNbcu?ïÓ|Çy°+?sÅÓöjÒ?gU…øÞ;?haX;×A?e.1Vöí?c¯ÙC…+ú?î­¥ø.w¶?¦7¬3iÕ?™ùϼRä?Ÿu¨ÁÕ¬˜?Qq=Þ%f?–ÉïžoÄ?î¯&Ûûš?›Ôÿ"Õ°?œqßòapŠ?'–¿(0;ð?Ÿø;2]?
Ê	4Ô?éЇ˜ûP¢?»W@rÜ^?ÄR:fÿ£¦?º*±-ª+|?¡®œÔLgG? »f¦Þ3FGL J1548.8-2250@u½¥¶™…@8*% Jù#À9|©žÊ[À;?fg=%û¿Ùà Fåu@'#C¦óÊ@b#¿ø¨ô¿ÙûºÁ1Ž¿äcíÖÝ?¿â¾ŽIj"X¿Õôg25©§AGNbll?ï[,'dg?–'©`Ÿ?i~ÆjA ?fúDŽHY?'h}æ¦*Õ?•!W§6nm?﮲¬!£Ó?…áçÒÆÄ?pEåžr?p$8¸—?x`Äߏ¤F?¯þª4§?íž3´®fH?ŸÍÂÎ[´?™ÕŒ,"ð?‹ÿYxâ'.?©29ïQ€?™:ÂGºt?í‹$pã?¡'?\­—g¾Z?`+äR›)Ç?³4&" ?ƒ? ê­<x3FGL J1549.0+6309@X9Àgn@EùJ?¿2°À:iêÝYÀ<‹?cÃÀ8‡Q˜y@›@"Yò@Î8£NN¿æ@Ç/ÿÌÿ¿ìpژ½P®¿ÔùT~¡4‡¿èƒdç"AGNbcu?ïòxv´f?jÈ»±ýNx?Aûî–r?`¹˜'åÔÚ?RFŠŸë?d«kbåHA?了<{Qƒ?W/dhåÞ?u7_?\dî?ƒ9·û¦?wk''úÚ3?'ßОA?îa}Ɛ?"Åíkó1c?Œ/¡ÓtÛ:?†gyZŸ?¢ÜGjÆ`=?{XŸ=-?ï%­¨$s?‡X¹.w‹ð?#góq£Î?88J$.?ˆhôÈ0T?‡9Z«óñÓ3FGL J1549.1-5347c@tuè_ÐJ0?Û¨h r2ÅÀ7p@Õ³%\À9ý"'¤?ò1˜Ä1²@ŽG…z©@xǟfb5¿ä̬¶¬Ï׿èD®?îØe¿æïçCp˜¿ïïå|OTHERsppa?
à51^-?Žéc;zK†?և}6¢Q{?πª4!çÔ?ä;ÒcLQ?ÏÀòJ~"?jpE©(³|?"œ>^'îï?ÛÁÃ@j•?Ë%1
Ÿ4U?âX¶¢?ËL«Xª¬?·Ã;û?¡áá'ÈÌ?֙Yhá™Z?¶ÜŽ	j?áÒðÓ'Á"?·c›[#?¡ºŸ™)›?™`*bz?Òv§?¿'ú·¥?åØÍSçÛ?Àð'¬iI[3FGL J1549.4+0237@%¸çÖyõ@DtÈßØBLÀ8j™ç2«À;UýgŸKŠ?ÛÑ^$@ÑIOL@´é •vÊ¿å;ßÊÞ鎿æGkX,€«¿åÉ_›'8:¿ë:ui0AGNfsrq?ïò†ÚA.?Xûù€U?JEkh,ž£?LQÜ^{m®?KŸ+"έÃ?M$÷"×f·?ïÆ4ñݝT?{˜þƒ<Rð?i@HŠs1?mZ^œÛ?pæììf?sÏ'wõ?ï!ó?‹=UÁa?‡/"‡pßT?}µ9ÑLߥ?Çò¸$ò ?ƒ'!;_+(?ï™6|CX2?‡?‡%Ù¨}?Tk{Ý}q?Yu;Û´
?‡$ñszEK?†,§‡ï3FGL J1549.5+1709@<ҏÃæ@Gç
€CRÀ:–ŠQýù–À;ג'µP¯¿âjڋə´@f÷ºâ±?þ¨›ÿÊ{¿ë;iå™CÖ¿ÙS'Bï$!¿àü¦Mÿ^½¿È´q'¥šÀAGNbcu?ïõ8ûÁe?82	=K?C?ÝBÍP?ucÒÝ¥kk?GÝã· S?'^ë/xn[?ïÏ:ԞMX?ztÚ-gð?g$iM-'<?p@"íN?i Â…?p<DËÞ(?…+ï?#áÞr2?{û¡#Y›¨?x
?š®€¢?ÀКm@?sø¦Qà¾?ïè‡Rdq?c$PÔó!?Z'³ÅÒ?"ÇUi{?gCQ$x°?bù›Ð}J§3FGL J1549.7-0658?ó˜OÌû@A¾ß¤?æÀ9;´L£FÂÀ;DD<oò׿î求÷õ"@ëUN.?þÇÑ`w‰¿ËðzÑØO¿àkI]ǟ¿â¨ëy5K¿ÌØ¢cÒ§AGNbcu?ïÀ4Í^C!?ž÷œí'Ç?oS--]?žà†M(úº?pYïºG©?lŒ´~ z5?ïÉLª/ ?zZí±¹[I?fMË
)?j ÑÁϕ?pMÒEcË?sóá‡ï¾?î!MZÒßÝ?˜+"æ8'þ?š¿ôââ?Ž~øëy? ‹šX`í?Ž¼»Þâþ:?ï
ùB"´š?©Š4Ti?5µuæ?@Aÿ·?êÕͱö?…Õy	3FGL J1550.3+7409@[8_á'p@B×@&`½À:oË
Tí˜À<¶ŸcÝö?á‹b¡àºë@¬P¥^ô­@›@bƟ¿æz\q½T¿î1=#:Üd?·ß¿¥"F¿ãìüÝAGNbcu?ï÷ÙÀ—??…aë‰a©X?L8©†¨'?…XDzՙá?!¸qdL?$š±¸z?ï­\´•o?ˆ¬ü6&¦?sØÛÃÉe?|
֜"•?uŸ5Éñ~ä?|@û%"?ï6èqS?'§©ÏÁ8¯?'K¾rg?‰yP8ãdÞ?úÖìǸ"?‡¨º³<â²?ﶱÛ?…–OÙv–¤?A;Ø'*?P½SšübÏ?j°	{¼F?"¼©O":®3FGL J1550.5+0526@,gÀ_A@EÜà@GÀ8à€If{_À;n"aKts?ílÂ|*¸@&wºL@¯ñ⢿Õ.J ã¿æáNö‡¿â$à"¿ïþÄö¶ørAGNfsrq?éêØ
'?À"ú©'&?Ä@6掓F?¿a6	/x? Q£•¥p{?ž€&4
L?ÓßSxã?ÉG+¸ÝþÉ?äA[XJFd?Ê°‰/v"?±Ý§ḯR?¯^. s½m?å± ( W¿?²uy·?ÊÜä¾qº	?¯ÄlïÉ°'?¼½5>Íö?£nÁéoÁÑ?׈3ë=íÂ?»òó'kÇò?Þ'LÊgüÉ?Áò·ên•?Ä þ"´*ê?³@pW(è3FGL J1551.1-5610@tae¿­)™¿ù­1@ê«ÛÀ9²`9ü{À:" z^jï?í·ºbM8S@Ë îؐ?ü ¢qON?ïwÌT×È©¿X3¬Äˆtr?‰7º£ÌŸ¿Öþ«OTHERspp?Ü÷+0"?ÍûN'~¾?§¿'ÕøoA?¥	£Nr?àq:uÍ?ÎñãHE)?ÔGdÁ®?ӛƒaB°?±~
LÛ?±ÛH}"š—?㹋õ–Ý?ÓGÒá×7?ޓ‹˜I?¶´B562?µè
8&ˆ2? ®ýç èó?ÛòqÙàg?¶POÂÎ?á±]È{ˆ°?Æ\±Si˜?œôܨûkë?£ùp¾VÈÛ?ÚÍö¤y7à?ƦÞàzÓ`3FGL J1552.1+0852@2q_¾¬y@EÓ7GMœÀ9õäžz©êÀ;¯%v²?¦šXmjÁ´@ÿ-ªˆ)Z@®{`sˆ8?'`ÏÅòàT¿ßŠµâ5ÐÙ¿éñ¡À¯ˆ¿àé¡r¹–AGNbll?ïRºfš3W?šã[Í­?'iü¢•?™dnùmNÏ?iõ´U|S?tM]Ú«?üÕÕ?‰¿Vy"û'?~,'û"î?€Ð´µž'?y×c™¹?{Ò·¦ÒÌ?íܨðõ½? 
‰ÊU"?£ˆŠ|TÝ?š‰k^Ó¢z?YÌè-³9?ŠzJà¦áº?íïˋ®3?¢4"²WŽº?•[ÑwÌï?"´®æzځ?¦U^"Î¥W?ŸLhöó3FGL J1552.9-5610@td•`"¥¿ü#pÀ\|À7'¨|‹kÙÀ:LÔ¯]Ÿ?Ö.]pžx§@}Ñ2¸$@@YŠ¿Ýw¨Ãƒ"	¿ãÎ6YXa¿âo¥ßøù|¿àŠÝâɹOTHERspp@?¸m¡ƒDl)?º~â Íbq?©;½}¬ªS?®ŸÜå/wg?ë^÷¼§×?Á3ÅFûÆõ?¦íÿ¶À{#?·Ò&è´6?́ÑxœZ9?ÅԉåÃÈ,?çp«¦lá¿?È"¾yÁ?ų žÄöÄ?¯QHs'þ?½ݗ<y?£pÅY©«5?æðü%g??².O;í!?¿Ó†ö¯Ú|?´eí@l1?°Ø…_8?­º˜á9Ü?éê~uG=­?»vcê*+3FGL J1553.3-2421@u¸ÚŸ¾vÉ@6Z(Àª'À9YêPkR^À;WªÒ§a?éwØ?á[>@½¸Ûÿ@<_":4¿Ì[>¿çÓSà¸ù¿ào ½Ëä+¿î,º~t,ÖAGNfsrq?î–70@?£NÔú®$K?ž,Ë®BX2?šÿ‡¤ªŒ?ŽœŸ+M?–Á;Ãw\?í}Ö²êwì?ª»±Ïð¤?©!­"µUn?ŸðÒÃB Ö?žÎ{FW?¢OnâïÏ?ê_y+à±?­sòN?½s'‹£ƒ?§9€pöª"?¯!h*­ç?žFiô]??çùd;#þè?­Æ':mý?´`>û'ª9?£x¦úd;õ?ÅêO•Ü/I?¨ÿ݈^Q3FGL J1553.5-3118@uieà.©a@15·?œÎÀ9…àãÛKÀ;Oûx±Â…?ø(0…ÙÉ5@>4r"‡>?"3/ë¹Á?éÇW±(Ó?ïû¡ék¶T¿ÓSM©oê8¿×æõU_¶}AGNbll?ãkI:יJ?ΰúS4†Î?Őφr¯?łVћüp?ÌÂŽ(&?ÐÓå°&?àõ?â_ï¿?Ӕ³¾[?Öã1ãÄí€?Ò'›eì?¼É9]ìÌ?ÀcÙ¤z}Q?à<2ö¶iÄ?¶ÊƬˆ†É?Óüê…5?µ¦qÊç)?Ç`$"†?³2>â¾µ?ÞÏI°äÊ?Æ|T3ªFÖ?Ú p5~ܜ?Ț&ñڝ6?¿@úe?½šq3FGL J1553.5+1256@7ɁOP @Fœ  0÷ðÀ8;‰‹.œËÀ;8±0?õÄ>£©½Ô@÷A\k»»@ÅÂnoI¿â]ÜT)¿ä")y1U¿ç+µª¾§h¿éÿì²£ßKAGNfsrq?ïÛ\ÎáÕ?p ]ȅ?gëÜ8ù|?ibÌݜ?Yp9Êg?YĆº¦$?ïÌÐñµ.3?zHF‡§æ?hÊ|9?o06U»N'?kCÎД?oûþ¡l?î7"«¯
 ? Ká@ìX?¡Ÿì1™æ?˜¬õ÷[
_?•Í'a»ˆ?‹~"f×à?ïÌ|ÒûšÛ?}PÛD?HàsÂ&V_?YžËõւ¸?v¥ˆ	íÆ÷?{ïH!màØ3FGL J1554.4+2010@@ÐÖ 2¥o@Gß<ã.À:E‰bÙÀ;Êô¯iåw¿ñSÀßIý@–Ehƒ@¢à?Ee¿æa‰iÃ	¢¿âԗ.Z[k¿×&;ìϿ簛µ
ú{AGNbll?ïڇ'•n+?'©#¹d¬B?YÑ+D€€?b+Q:Ëvš?hçÜo•?n_ð8cÏ?ï]ø–»?•Ë–‹è?‡Ü	uuUî?_{lÞâ?€¥ó‡dûŒ?"+¥·-y•?î¤Þ³ãæ?'¼ïJI?ü\zj~n?'—Ã
Åw?œeÿ¬ND?‡õ°êõÞ]?îÚj#d.5?"$ˆTX-?eŸD°b¥?j z…?¡3Õr?"eŸÆ+½3FGL J1555.7+1111@5ë€uf@EúÕߛªÀ6‡ÜŽá¯³À9Øoàb«Ç?ëXlQ?–@DGw7ïÛ?øO÷øµ¿Ñ$¹»Öô¿ÚbR'¿Ñ§—U"þ¿ÑAЉ3´§AGNBLL?åT""€÷½?ÐÔúk?}mB¨<BË?"ÔF5§?ÔâÌ]|?иÞÒ>Ðó?*ë<:‹?€;"ÍYùß?qï}b‰)?u`ûBOÕ?o–ÙÉb"?s	ÞO¿S?ä2CY"Œ/?·WgÚÊ?§7;PZ/G?O"–|Ë@?Ô´'âÍ¡¹?µ…*¬¦Ç?âZ¼zí†?ÂC,ª·?m¡Pñ¯l6?v·þÔ¹t?ÛDhA"*?Áô2SIT3FGL J1557.4-7040@sÓIàâiÀ*QGàiaÃÀ9²ªÿ«1À;¦™_·öÀ	)^€"ä#@çÊ´èª@h(ÿӊV¿åx­Áä}¿â¿"nÑ3¿âÐ*æô¿æg¨MðŒAGNbcu?îú®ŠU
?¦>XVìPú?vœí—|?|W¢ë€?$?›99‡yøÌ?¤Æ¶Woh¾?ï¶|š_"?Š# Â5X?Zò‡1æ?c#W7@·S?~;7
1p?†Åäaj¢›?í€ØßØs@?˜ä$Ä~?˜Gbgœn?…3…b?«ÎèQDýÂ?˜:¡C¨°?ï¬ì°¾;¢?">?"Åò?÷¢ }?b¬­¿h—?"°¾Øñu:?"8Ò8Ì3FGL J1558.9-6432@tøŸƒ¾fÀ!GŸÕó½À8ÉÄ<ÛR¢À;@cÞÌ©'À¿^\¶@fƒÂ—¿¥@0K`{•Î¿æ륙=dv¿Ö†§qüû¿á}PPB¿ÕÚiýc‡SAGNbll?ïÕfu}?nÕ¡^v#?I$7¥"H?HÖv`ž?r* º€Mû?l§…^1Êà?ïãþ'ýk?£af©¡š?e-(ƚ"?tž.e§"?š•çr?¡®Æ3:²d?íö'_õ??šÙD{¶I?˜ëFß¡¿?Š—+e¸?¤!FÛŽ?'òÁÓ!Ÿ?異³9Û¼?'Ü®ãÆó>òÕêb'‰?
¡¦Åžw?†è<W¯Ç?'ف֯}3FGL J1558.9+5625@UäÉ$.@FàxÀ>-À9DËüÃ4žÀ;´Sø¥˜«¿ñmš}[F@éÊ@®êÖù¿çè(Z½ë¿Þ–÷Üá¿á·_öW,¿æŠt¼P¹èAGNbll?ïøâz.Y?aÆë‡'†?+ãSì2|?'85RÁ?E~ÅDŒ[?a«ÜrÁC2?ïɗËîòq?xáêNWé˜?h^hð{q?lRa¡¤Q?n
'¨
?o¤Ñ^L3?ï;š–ªAá?…tý"?'M—‰q?bX€7}?ŽËÂËýøŽ?†ô=z¹Œ?ïÏÍ6oµt?v0õޞ¯?2Ü®úS¨A?<ª÷H;Aä?vë™Ø€¥?uÐ͋¡m3FGL J1559.7+8512@]·Êÿm3	@>TDŸlArÀ9ŒO"}ŠÀ;䰔‡áá¿ða5Tu£@{=gµj@ϊ¿Œƒ¿æØß/®vÿ¿åõ³ö3šÚ¿ß´2¿o¶¿é~ªùF&AGNbcu?ï×pºß?s˄æP8÷?a,›a˜?a1YÕ(r?gmbªÛ¾ó?n`²q…áŸ?ï¯(‰jëÓ?¦Ø»UŸÞ?q¡Ô¼ý2Ñ?p46W›!?vÉ捌ä?{ñ,Üð?ï!µ7?‹Ëdèµ?'P¤)zŽª?{¦uCR'?'¶G¿±Ú?†.֎ÞBv?uՈ?‡~Vš£s?Jሆuö?V𱥁U"?ˆí
2£>™?†áŠ(ÑÍù3FGL J1559.8-2525@u¾q'l@4'	€²BÀ:lÚÌiÐ~À;ž
ø†¿ã
U€1‹
@€wö[¼i?ÿ-€kË*¿éäåŸxù¿å^â8³•¿ãK±së?­-ZoüÖïAGNbcu?ïñr«ž?\ÒËjä¡?48Ê·ô+¡?2Z̤²Êw?X
§$«½¸?Zê'3,É/?ﲄé¼Í?ÁµF[ì?j†3'»·u?tÓl?©§?yzqX»\?‰ô$Ié
?ï
Eo½?…)Á&Â?äߝ	Ù0?qŽ€ÌT$?•[‡ƒŠÛÆ?'ז …ç?ï?[Pι€?"-Ðt¢óÞ?1¶bæ‡M?B°m4a-?—ÎW5Ý?"'þñZ½3FGL J1559.9+2319@CTÇÀ'á@G¸b`GhtÀ9玦 ™À;›Î­wœð¿â"'p³v@µ
eÄ*@ÍÏڀÀ?íÂÀÜÿtë¿á-v"q¿äPcxSŒ¿Õðï
(;ÍAGNbll?ïÏrS¨O?©Eøñ	?anÁ×19?Œn×÷š>ð?oŽÌ€?¢1›øzg?ïÆùòCl2?}F^¥žÖ?lÁñ¿ëù?t€[–Õ>?lDü¨´È?pžaE`µ?îðŽ;X»?ŒY k:\?ŽÝ{îÑÞ¸?ƒ–ü2mÁ[?'~¡+ù8?€ô…/²•á?ï5û®ûÛ¹?" ëRßs?S.îŽ]!?Xn¸?˜
›7ž¶Û?"Ø"ê"~3FGL J1600.3-5810@t\3¿µÀu'1>À9ìæ˜Oí~À;KRü&V¬?áE'ÏiÕ@	d^¤P,@Ô?\â.¿âÌ Ë¸¶Ñ¿"îj+lë;¿æ}†Ev¿àpLžÀ—AGNbcu?ç3ë]j5?ËØ?ß{?"ǁRÂ`?&³Jû?Ð[±0
o?Ëlñ4WÄÑ?Æ,"±¥Ÿ?Ê ž…{Ó?Ò/Y²ÆN?È=]ÌpS¬?á].°o?ʝIP¿I¥?ëò·i‹u–?¤³Iܽ¢?¤Ê5!_B?'g¼èÊ4?¶*"ôЭ? ='Aå/?Ú|]ÅÓà?ÀX±NÔó«?ÔLECM¹–?ÄŠ½Êٞ?Ñ7]§ìr‰?¼ãzõ‡|3FGL J1600.8-3053@uzÿ°Nè@0uS€°"ˆÀ9Цã.8À;É,.\4?÷>¸ŸÄ+@PRþª•?òšª8"[J?ïþ+«™:=¿Î²¢¹ÑB¿ÞTn#°¿ìbÇÒßWáPSRPSR?¤¹ 	1Š8?£%Ð@{?ëÇ>"h0?¿¡B}?·i;Ø%ºT?¼»4"ÛQu?¸"úЦü?»œµÔ'?èmØøº«?ÄÑPßÕL?Â	
Ÿ¯Ô?ÁGb—î#?Á[~ßi7?¬…5¼%GA?ç°åfWhT?µn·OÈé?¿Á×r¦ó?­;ziâ'?Ì¢O3¢Qê?·é>7·??äp»c"?¿Žf}Aù,?ÁuÞÑm?³³Óô¯%3FGL J1603.7+1106@7ôàM/@EfÀ(yœÀ9ÑøQÆÀ;{Þ-G`è¿©­‰ô1«ú@,f…›
@˜¿aÕ2¿Ïû/i¿æÊ-ªL0¿ãÕÙE"–O¿âïHïíAGNbll?ïðÆr©V?^`oÃ(¢?CQÂIÌ»<?Kʬë_r?TÊãõÆ÷‹?Y:"ÿqØÛ?ïÄÑé2¼€?z‰Œc‹?ltuªõ0?pÓ­ê•
é?n¹¡"Nl'?p'ك¶r˜?ï(c&gV¿?ˆ.±	Ü?"Ó_
.V¡?yí«šwB›?‰ë­ýüÜ?€±´ä¹m?ï1ÉÆAÞ?‰y]LXóÇ?UµMákaÑ?SçÜ.²Y»?˜±é!8?ˆîƒJý͝3FGL J1603.9-4903@t™€o&)@Œn¿{UŒÀ6üUFƒrÀ:Vól|*?ÖØÛ~@w¿@ˆY«B@«ÿøž7¿ã\̀—¿ä©a÷}
Ô¿àš¹yÞ¾<¿Û+I¡AGNbll?ë'ºƒxd?Âù
Í5?`#ɟE,¸?`rX´‡?Á·ïu	¿?ÂäžÁ¯/?밊S›v6?ÇӊÙ7¨?zþ0¦Mß?Œy?;ògë?ÀlæÀô¹?ÇM¬uͱ?ãß4K	vÖ?¶À"1-Õ¹?£/˜…ƒ0?"ÔXÓ%0d?Õà±vÜaî?µÂ‰Òü?íu{±«f?¤GV—³B?8¶¥v2'?DÅN¹?à?´;q,üž?¤9yp?3FGL J1604.4-4442@tòߋr@|€.8£À7µ"k4+À:ÃÝo²?ƒ?çðû"'\@7£9€A@Ÿ­@j~N¿ãª]ÒÝÍ¿çå)MèQt¿ã–È6¿êÔí¢QÆiAGNbcu?îdÕëZ?¤Öþ¦úʕ?{ü,<.g?{Sjp+;?¦3È/Dx?¤FŸ!Œ?î™,Äü=ì?®³Z3X¾?kºM#]-²?qÊ-U??¤±ŽÞNi?­Ç°úø?èÜýÕq´Ö?±·¢)£o>?°\˜N÷??ŸÄÑ⥅?Ä]¼'½?­6
Q''?îmóX,­t? `J" ô?[5ÓJT\g?^?÷ÍMa£?¨Gââ…Ñ? Cð›Cn3FGL J1604.6+5714@V(Àª'@F]K 'ßÀ8¦'w"ŒÀ;'ìÝ
?õ"AöðaÒ@•‡û6——@žð86Ó&¿ßŽ8	¿ç?Î)̵®¿åò.XŸ¡¿ë{ùJ¯&AGNfsrq?ïá±?d܎³P?eE3rÝ$J?^¸çÅ'.?S_c㭆?VªF"Ûã?ï²DÝZüÁ?ƒ"%"Cq?tȈ÷c*/?yˆ¦à-gw?r[u'?vÜÆßç\?íFN\/þ_?¢Ç x'õž?ªÛùã{,‡?šÕ+2Eý¾? ¿ Y"íŸ?")£ á¶G?ï-(uŽk/?–>w381b?€?è"ßϦ?6p0R²[?':ý²F?"J€â"U3FGL J1606.1+5630@U̚ÑVŸ@Fdä`gHäÀ:~À?öÀ;ë¼Õ±À $rÑç@Þè<k?ÿ'N^²½Ø¿ã«;þ'sŽ¿èbÅ'øþ•¿ÜÄò]€
׿ǯLý£sAGNbll?ïÛXjœ?y©"@¶$â?4ÊT?6(ÎÚ³Ö?q4ãjé?yÿVUí?ïÔØÇtæõ?v˜-&þéÅ?c¥f×`'˜?jc	EO¯?gÑ³¸w@?m©,irÄ?ïÐí¢±?ŠeÍqŠ?€PÚS£+¸?qÂAæ€?—µ¸zû?†M¯y?6Õ?ïê\¹'XD?d«d:I™|>̖VT	u>ß°s"í'?eœ Ù»±?d¨,FQ[Ô3FGL J1607.0+1551@=`A€ÓÏö@Eµëž*ùÀ8kğס<À;]_Âví?꘴îDýÇ@çL‡`\@F¤‹¿á—:2›¿äE0X.ã¿äñšÃ‡¡¿æB7Š°ÈŠAGNfsrq?ïb^YtÌù?×''›‰Ý?‰c	a"Ñ?‰í§gñš3?|
Á<Ö[æ?yS¬''è?ìbœÇ'?·H:½&¾g?´Æ•§ª:?²¬VЉCà? I8äÊ?£ó;Éo?îl
•m?œ Éúǯo?—zxPËi?DÈ!‰ ?¢Œ.¨Èô?"…áÿ3É?æpP¢]Ÿ?·Îmœ\8B?ÄÀp'0Ê?´9Û«'—È?Â*ýRå?³Ö X±Ýº3FGL J1607.9-2040@v, <K
@6""?À9½¼{À;bYG™ò…¿'0ÖÔcø)@
c-ÜÝ<@?©c;¿Í2=¨4ō¿àæNè订¿ØØ©òçz¿ã²öЉùFAGNbcu?îöãs«'?¥:ó¦s‡u?v& ]?réžä¨i?›ŸU†rá?¤>¿gש÷?ïu0÷«Á?o¥kYà¼?€wzU4?yˆ£ô¸
?'˜+JšºÐ?ŠiÏMxÊ?î
4Éûï ?˜×ý'Ì''?"îîñ˯?"w–١˨?¥ »èÈ 8?"ºZ¬NE~?ìg[ÔŸí?Ÿ%>ñS?zÛ¸ÇL?u§àþ…?ºÍs®·t?žké÷ƒ¡3FGL J1608.6+1029@7ÿ·ä@Dh _ñØÀ8‡ôafLeÀ;\¤£¸×M?ôXO´HG@_óWûêr@óÑ@yí­¿æˆ{QZÁ¿æû…å\»˜¿ë	Jƒu¿í¯|¯AGNfsrq?ï×wË©ñ1?td<À³?qÏYë'Rk?s/ŸZí™þ?C¦û¨ªù?Já߈*çk?ï{€Štø?Œà]@±?'j¨X:‡?ƒœàä‡Ü?}jŸŠQU°?€ùb{†?îE¬°Ò…ƒ?š«°
Å ?¢É‹åáܸ?•Ìr"¦¦â?'·Rë–(?ˆ
ˆÄ^C]?íÆ&=^'?¥LÏø=$?¡
€Ê¨eÍ?ž·ò?¢"_nq;?ŸÝªÔìêB3FGL J1610.6-3956@u3¸Ÿƒ¾f@ þ{ßõH—À9ä@†ØÍÀ;
þ®Ç(?Û>ëÙÛ@(¬~¨@áé€aº/¿çþöjªï¿ét¢ #¿æZ||¨¿ë§"÷ 2zAGNfsrq?êAÒ=n°?ÁŠß1ؾ'?¤Š&ÄÄÓ?¢ÂS%G&	?ÁÖ-Y\?À8:¤|k.?潈ªö?ÈwâVwMw?ªÒÛï§É?§Ñêˆ\™?ÎUY°íj:?Ɓì¾p9?äSž/×àˆ?¶bŸNÚ×?Á
ivï£?¥'g•ø?ͤÉ°Úà?²<éôo£?âѓ|.Ûá?³
»Yòj?´WycՇN? Þ3áâÑ?ÕFú®¬æk?³œo½ÏDe3FGL J1610.8-6649@t™÷LÀ&J§€âéoÀ8[#'Õ€À:ìHŒ`Ì?êm¹'~[6@¤­ùwû?ü^¶­yö¿ÜxŸ
Î2¿ÔwFÀP4¿Ú»¼œpR¿Ñ3þÜáº<AGNbll?îß>0=AÝ?§ ÇœÚû ?cæÎ×2˜ø?k#}†ä"å? Í°¸¸¬?§#;.¥BV?´2…?ª¹Çä)ˆA?}`VÏ+ú?‡¨¿«Ú?¢óx±ýÉ?§}?= —¯?퉝²ôW?£ÅrŽ/Ï{?—<8:?‰¼…4Bü"?²6¤&O0? µ­×jjN?ê¯FÞÀ-1?«€åÖ%ԙ?€ŸcyÔv†?ƒ)FFû?Ä8îMbÒ?«-2A˜$³3FGL J1612.4-3100@u¥ 8L@-JÄ!, rÀ9ÌÎFImÀ;—A¥Ãt?öCÞâ# A@"1jÜí?èÆ£É&Ð?ïýϘÑj
¿·l'ðû!Á¿ãÊ"Cñò¿åàÜ+íøAGNbcu?éž?ˆŽ.¸?Å^ýX'(°?¶pÌX$u?º'æ3{ë?¼ãï6eÍ?Âÿ'ñ™T;?èP…Õ?ËÑhØ.~¢?·©G!m?¼s¹g~Cr?Ãó[-`ñx?Å͊ㅞâ?âDp"îÀÑ?·;!º«o?Ò};	õ6¹?¶NÌèÞ6¶?ÁóÉ`ZL?±.2ɚÁ?æ{u'UE?¿Èèﲓ7?ÆÛsêæ?¹ÎÿWF|?¾mlQ€×?¶ƒzK7å;3FGL J1613.8+3410@KŽÀA¤@G,|?ìÀ9…'Uþ9VÀ;ۛárv?¿¯½_ïð7@.ƒíŠÝi@Кßê¶Ã¿è$¤ˆœ,'¿áÂÓþüR¿æÎPZ‹¿ÜÌñõ-xAGNfsrq?ïs¨=é?"å)Æbf?…Šëa
oo?ˆs—]!\?{`U`«ã?ŽU…	ޓ?ïm\ƒ½Îb?"‰ÜzèZ?…z¯Ê]"?-ƒÎ?~\^Œâ?¨i¡‹?îY¿¶sÚ?˜ BÌ^4?"çnÜAMu?‰pj®í.š?Ÿõ,ð7`?©˜ß²?îÚûÆñܝ?˜x¬üçõ?ƒ´‡¸ÀPý?ƒ;$p¥ÒQ?šÆCEdCØ?•%nžbÂ¥3FGL J1614.5-2231@v	ÄupÅ@42«@‹
‹À8z½ø³oÀ;;…Ÿç't@Bv½K¥p@&©fÁ*,?ò˜(Ë{>?™È—«OF¿ÅPVHzÜÚ¿å³ìí\[Ü°×PSRPSR?a'w=–¼?`Ø;|$¿?ï»úށàp?‡Ü™Áë?yAU D¸Ë?…ÿÌ󒍩?rRÏsXQ?€Î)9l¼,?ï/M!âáÝ?'V¬oÍ?•¨ÆîE?šÏ¤œÛ?–Ùb:åv'?ÎӇ5é9?ìê‡bƒU™?£ö(<uê»?²õl]+õ?¡Jw
ý')?‰Æ–ÓàÚ°?¯LÁh?b½?›ñhb»Ë^?éSÌúò?—2"ËlÒW3FGL J1615.3-5146e@tº£3v¿å‰€5´1À6ï¸GʐÀ9»–~\&r?ï$&O­@þ°³¼…'?ýÔ]àZô?ïýßÉÿ'ó?"¬'ßZö¿à'7'߿ހ¡{j×OTHERspp?½ß)+èhó?¹hR'Â?¨VQVÄ{?­÷ñA]c?êÄum†š?ÁA±SA?¬˜fÁ
Ê?ÀÀÏ,Ù?´^nÞÔ.Ô?ºËuJW?몫Ã)iJ?Å®LLË"Q?ºÿõÈÕr?©2BTÈ:ä?¶+€§k~'?¢ÅéÏ3ö‹?éøoìYu'?°Ã/@(R?ÂkÐUjj@?¸<ÑNÇTS?·J·Ô¤Á?²'÷ÑF?è{µ
JÐØ?¿ ³"sÕY3FGL J1615.8+4712@RwïÝëÙ@FË/¿á+ÿÀ:X¤ï81 À;ìGJAl²¿Ë•ÌŸDB>@@q@)ªo÷µ?ïÙÖɔ£¿áòT"¿ÜÚòaSN~¿å=†uûYÓAGNfsrq?ïð}ÃhìÓ?U¸Z'³à?M8–$Z²?M'€¨"¿;?Ph.¬ ?J
:Ç—?ï£ÄUÃ?"øcX°ƒÏ?y—Xê"*ù?P¬›Ó¬?t†¤jšS?ul—	¿?ïEÈ;êäÜ?"oKÌ¡²:?ì댛áp?vRô|à?Œ¡xªça?|
d‹‡F?ïV?õ?—º}¬˜‰?rîŒ6N?o1(Pz;?›#œ‡¤€¨?–{Ò#•k«3FGL J1616.2-5054e@tÅـo&)¿ÀÈßK³À6"`4óþÀ9ákÀB{?·ä»uÊM@ÖSI3¦@(ˆ!ö¿áí¢F¼¿æ‰u_'®¿ãg–²^Œ}¿ÝÄ&¤`OTHERPWN?²KŸy)E#?²U¾2\†'?Z#b¿°á?_i—‰Š'a?í©z_zþì?²Š–¿e¼?Ã%£ø	ø#?ÇÏvù'ÁÐ?•ò\h7"? ¨:"Ãà†?ê‡!Ú@;?ȋˆõ§¼?Ø_*˜sÁ×?µS,µT,ö?¥Pˆæ?–b…œ©?â{j{7½³?µ‰í}c¯)?áRv_;"¯?ÄØhUD\ ?BÇVî¨~t?KŽ·S@â?ÝQ¯–'a?ÄÖӊ\š3FGL J1616.4+4631@R7Ã_Ñ ï@FÈûÿÀ? À:=aŠQþÀ;סS¢>"?Ù©¹‹Á-¡@­N€@­@»0à¿éaˆcÄÔ¿ê«ËŽå¿ä֌]é6²¿ïÿس"smAGNfsrq?ïö1C•u¬?yúÎ;n;:?1~×Ozã?=1?ŸN³?N{†[?yÒóÌÛI?îÙF—?¡ís˜GtQ?˜9
}àî.?êàMuþ1?‰<Jžy#Ò?ŠRŒA?ïHb/l;?"«*'}Cž?…¢õá3›T?|o°«*g?ˆYq'ñUÙ?}œv¾»Êq?í¥GQ/¸?¡˜&±çq4?¡l;¾=úJ?"s2ôq?¤?O.ÈúB?˜07ŸQ3FGL J1616.8+4111@PP9ßõž}@F÷¹¿©Î›À:"~êÁªZÀ<o%QÉ ?Ùf¯"ù>@Ù§b/'@ ™`
Ü·¿ã—"%ĵ§¿âP'gñ׿移*'¾¿ïÿWZýAGNbll?é¶W0LWv?͗3N5?ȉäê?ͬ3^m÷?€ÙûN›€³?€µ£aˆ?눱6‰?¾¯ê!Ñc^?¾¢+Gܱ?»ÆÓ3Lµ…?¢¼´Õ? 'IhÔõ?ì&¬,÷?§_O÷D™¦?´^4J(_%?£ݾ­‰k?¤ØÖèï"J?'ÀìQ?3p?é*Ú¡0a?¶^½"|%?Æ"á*`A"?´ÿ:Ögj?¤ÆÑC}"Õ?˜–»KÂ3FGL J1616.8-2300@v	é€,
J@3w›ßÄ÷À9¼6YX`êÀ;73Ëßg?ìN¼9'Ùó@:zÅnÇ@Ûÿo·H?ïŠ3•XÂ9¿çŠ"ƒÉy¿Å7&‡ÔQ¿ïÿæPlOTHERglc?íNH¾G«?¼YªìBRÃ?©,Þhô¬™?³éFw&?¡ñM&ظ?°4¾†+w?èò!½ƒR?ËB¡CI?ǽÉ|z¢"?É¿©h¼?¡ßò=@›?§ú6=*?æ:Amú¦<?²èŸk?ɕeÈc·:?¯÷$ZP"<?»(ÿc_©?¥k=ŽÆ½?áKl•?¼þ!ª2»?څEÖè›?Àu
ڀ?Ô&Z;aŒ?ÁÞx6۞+3FGL J1617.3-2519@uî{¿"ÿ&@1Î9ßõž}À9(>Œ,ɍÀ;ç½f?ïÜÙ¤ƒ@
Þô¾@¹³ ©BÚ¿ã¥æÞ4Âï¿ê³'ɮƿåOI¥v®¿ïß²Ej æAGNbcu?Óô2'»9º?ÇÛA#µ?ÁÁÓ*ydX?¹õ'p¹Ï#?á•qì

?ËÂä‰
A?à4<û;Ñ?Çÿ–ɍ?ÙZ/…Gn?Åڑ±DÁÙ?¹£éZ¸?´B«‹Åh?áNB l?¶Dì"xR?ÇúY©?\?ª˜®?ÑfO)y"?³ÎYlT‰/?̬ÑŶL?®´!z}˜?ÚM®zÛ.f?ºPW0I?×[袣vu?µq7Ek=3FGL J1617.4-5846@tp/hیÀ'ò€¯ËÀ8pº¼ÿÐ/À;I]A#·?Þª¶þÀv@n'!€-b@Þæ …Üx¿å÷ŽÔ'É¿èb¤‰ýè¿æ¶òI¿ï"äå-§êAGNfsrq?ïÍ]Ùj`M?s›ÿ̓?b´‡u"ˆÄ?d);"=V?oíŸ }+è?lōΝ¡Ð?éUyZ;SP?É[õÑ?œXGN½? ÁÅBÚo?Ç&")Èê?ƪ•&ǟ"?ì™w,…&?£iú_P«¶?¦ÅaÑ9f?"Î[°L?¯£t‹ft4?œ›Ü,í›×?츠Ëí+?¦Ïëg
љ?Œ‹b¥I?‹¬¢vøk ?¶©•ºõaô?¦]Ý~Ý3FGL J1617.7-7717@s–¿šÏúÀ2Ûú Âî'À8ª$[ÿÛÀ;b!¯é?÷whlP
Y@m¼Æð?@LŒX¦¿âËo2F¿çFMqj,¿ëϋó¿íA1×8AGNfsrq?ïšÿ=?"éå#E+º?~ɱ´Ä3?|Ɩ+3J?t'j΃…?tøFhsÿ?ï08H³.ƒ?J*átA?z\¼0¢ía?'Š|s`Tÿ?"aÇÝqtZ?˜¾×x‰¢ ?íépêÀ'€?›ì™Æ¸7?¥š¶ü+ï?"ËlÅûÊ8?—œt¯Þ¸?Œ¾é˜ƒÍ?íšìø(ñJ?§~m£é­,?—þ7¦:??•ìº'Dòè?ªRªlÎA?¤é¼ç3FGL J1617.8+5137@Sûݿη‰@F>'_ÀYøÀ9ÈÉu)wÉÀ;ýåÑ÷?åÏòª""B@‰Ð2
@—'ÀŽP¿æˆAÁ!¿é¿˜ð°¿ïÛÛ3©
?ékpˆB AGNfsrq?ïúõ´§{ð?qz<j
?@ˆÌ™f%Î?qr_"otw?EPç?$D,žª>?ïËàÙµ?…©h5§?iŸ
©´+?ÃТáÚ?j€è=–'?qWÓc¤?ï`§·`œÌ?"ÆsjD½ñ?{ÌúVŒ?v}Åkfe?ŠI+ªÌ¡©?ŸXï "í?ïõ¼¾k½~?d!~YN?;?:¤¼'¶Š?(U²"ã¶?SŒ®£ÇÃ?cý|²p³3FGL J1620.8-4928@tÞUùµc?Ø°ä_¡·\À6o'£+ÓÀ9·i$†È@þÊéG×°@
*Õô"»3?ÿ´>%–c¿Íóê:zG¿ß7åKÁ¿âƲ†@¿ëÈMt…–‹PSRPSR?*N`À?*ý}¯:öi?ìg¸Å½ÁÆ?Àɱv‰ò>?¼µ¢îë?ÀÆJap{Ö?"®™[ƒq?5oõ֛b?í=—tëý?°®^èÎßv?¶	ðT‹ò]?°¯·)
S?u+—Þä*?s{eÊ à?ê¹kD?³ß}VÛÌ?ÇG¿fÿ[Î?³Ÿ'Ü")?E>BÖ©Õñ?DL÷T€7?éòI˜«Vß?¶[h추.?È!›Z{úª?¶Z±sƒ3FGL J1621.1-2331@v'Àa"@2fþ?5ŸõÀ9*Et~WÀ;+Ÿé>ó[?úxÏ>ìúÀ@:Lj'Ä8@¥e;C"¿Þ¶a$vñ"¿éÆ»£"©ó¿ì¸ï6übß¿ÞÒ¶õä·êAGNagn?çmBu'7?Ä:uLÚð?ʘ¯­U'?ÂÌ3ÏžÇ?°]ôŒøÃ)?®ê´S½'ï?í"h­IÄ?¼<a!!Çâ?§k.ò9†Ç?³~¥gõ[? NPñÜø?¬=kK	V?äcä8Üo?´•2{ZΏ?ʨ:Hm‹"?°PZv³ì?ÃÈ4×w¯?«ÃÉ@œœ¬?ßùÌ©>'?ÅÛ1ROd?ÐRgòˆ€—?ʘŠ
x?Ïi.œÐ?¿'…='ä3FGL J1622.9-0312@%"¿ª¥[@>¶ÌŸóPÀ9PAÌS*IÀ;cÊõ\8?ê ¨ÍFÍÍ@
Ãt±­·‰@ß@QSÛ¿Éxà^*X¿æ4ˆ1ߘy¿Ýx(ïý\¿ìâ.w¦nƒPSRpsr?à»Ñ(,\J?ÇÿÒøÂ?Òçìta?Äb†lºÑ?Ç@âvŒl¥?ÂBý[›?ã'·Ô÷8Ë?Æ:Rª-?Õ	Tq`Zv?ďk·NC?²œï'ÄÏÔ?±½Öõí^U?å°Ù¢ªÇ?²àµ¦N?ǖB,–f³?­>{»0V?Á©VlÞî0?¨f=¨k\?ÝL½ý.Ë?´:
*Æ]?Ñ£Õ±ƒ£æ?¸œÑóK\N?ÑlQM'?±¬ñ"¹@3FGL J1625.0+5651@U¦J`"@EÿÝÑÀ:•é ÀièÀ<­2ӑ㿷@X»§S@"x´q·'@+¾aO?ïýØ¢1Ýb¿ê«»ú¹çd¿àgªÝtöÞ¿ç³Îߪ'ºAGNbll?ïÆU9· ã?‰ŸàðIšŠ?q;6…l?†ÓŽdsSO?g4Y
Õ
?q¹$žµŠæ?îð'­X>ÿ?›»'.Ó?"øSÊíó­?""ÑCFx?ŒmXÌ?°îw'?n?튮û]?š«ë_·Î°?ŸœoˆÖ?'ߟ‡¸??§ÇÂÅ»ç?'7áíYC?í*\*[ ?®n!«Jlö?š0²ÌÎǛ?"/`ïK~é?° îËyq?©ïõ1¯¢3FGL J1625.7-2527@vP +"@0Ri¿·:"À6ñ\°Úþ¿À:u6xbm@O( °z@ðõ£ÒM@ÑBG£,À¿ßVàßØ¿å!¥øÞ´½¿æKf©¾f¿è«ÁYŸðAGNfsrq?ﰕš¶x?ŠQªf¦Xp?e}3Ù1?qƒú(nt?|öÙ%žW?ˆÏCª…¹?ï·W¼¼i?‡÷0S±t?cû¶G?iHNgÃn?zV•þÁá?"Ùµ?+óo?êœ-(¢4?°ÁX.u¨?²i™…K¥—?¤C@\3F
?¸´ý5£ÀÍ?¨Êpshž‰?ïy£wà?•m*·yz?TåÐÙ¸Â?€²ôȞ?#Dø?"4?[~/B3FGL J1625.9+4125@Pa¾À//˜@F@`B_÷À9Õ¢"›À;Îï@4£¿Ïk¶g/º@'G¡)Zí@›ŠË<T¿äoG¬DŸ ¿éÔìò9Ì]¿â›i+Mò¸¿ïùÿ•¡èHAGNfsrq?ïï¼&æ?aÒ[uoÖ!?=½‡\#Ó»?> Áâê5?YQ¿<?`Uuå_?ï¶h°Ê?šÝ`(>á~?'Ç.m3'P?"›â%"Êz?†"ù˜Èv?‡è°›[?ïFîh9–Û?"U¸*:¤?"4àCDg?t˜tþ–­b?Š…®V<ó?}
D?îuepß¹ê?œ:ök˜R×?¢èeˆÜ?‰?šVZ}?¡@îØ¢_ù?•êÙ×=4«3FGL J1626.0-2951@uÌó S\ž@*¢:Þù;À8>þ½	á*À:×Eßaô?÷¦g½ÿT‰@ Wš»-@IA½d¤ð¿ÜÕäÎ _¿è' +ø	¿äˆ=H,a¿ï	â.*W9AGNFSRQ?í¸BÖwT¾?²Ñø¨l^?™<+¥Îñ?›R+­[3?§Ý̂·Ì´?°Er_P??æœà^PÑs?ÇIK;›óÇ?ę¦¾&.?½›'¶÷cc?Àò×È°"?À½"4߇?æ>Þ5dÏZ?±îxkû Œ?ÂÎñÿ(»?©xJâÍW?Ä5–m™Ý?¬­û¢J?ܧ£Ù¨´Á?·$ùd®q?ÌpÅ23Y?¸ú1e|iÝ?Õù=ž´?¶ÂXÕüí3FGL J1626.1+3512@Lr"_õI@EôŸëWÒÀ:ۃ6€ÅÀ;ôyŽaW3¿èb‡Žv8@|¼êº?û2ýáAÎ׿ïÿ2Ìʸ9?ïýíXTø!¿Âs,·1ô´¿àÅÙ=žqAGNbll?ïüž"âÿ?;ɺ–6¤›?.YAPìw?0Ćý³GG?'¾p€zd?1'zqÕÞj?ï¥qºab?ˆBó\ÏŠ?x€ßМ^Ô?ïeÝ?tƔÒ2ð©?}9au"'Ì?ï)Œ#Nl?Š&y¶.'?‡—û'Ü? ­hýŽÆ?Ž}_0ú¥%?Å|#xÙÒ?ï͔۰ʞ?{ëzÄKzà?_¡¸Žh?l¥Ín¬ëB?qMKá,'?u¶©‡÷3FGL J1626.4-7640@s¤*ÿójÆÀ2Î_¿ƒ8.À9ÜKŸ:ÃJÀ;'"e'¿ùS)ÃGèÍ@+è«ûpú?ÿØJ^Èã3¿éI4'ª-¿ÔNd8Üü¿â‹&9O­¿×òÕÒ|["AGNbcu?ïð¦"oܶ?W¸æ
zG?:M)q
o?6 }æÑ|?X0ÕêQ×?UºãØ("Q?ᅲŷdƒ?€ÌÎþg4Ò?UəÕ/<T?] 	IÞéD?zÁ¶¯ðg?}©þcL'd?ïœ}Iq?Š	ŒHw[‡?…þV• ¬?v厂
.ü?"E†œ?Ó".–p?ï³ü%?xá¦A¤Ï?]Iá·x?æ´Úcº?ƒ'c¬ÚQ?xÐ$û©¾é3FGL J1628.0-3203@u·(€QÉ÷@'½ ‡_À9"éû±¼¦À;<êºô]5?û"á·©°@a&xº¦Ú?û ¤†_¿ÀñÒQ{Y¿Þ‹·½"k¿ë"Ú±¿ïÿexª¶¢PSRpsr?'uºOuC'?•\%ç¨ã?î=y‡_)?³‡ÐÆ7z´?¥'K?Ïkª?²g:íTš?'Úªê]6¡?"h×WŠš?ëî[qè½?ºî @'	?»Ö}Ùle?¹žÇ;ðP?®Í?OÄÌb?š˜˳™?ê;©(ßë?«c"yTê?¾¼^֚|?¥'÷#cK4?¤­©Æópj?"?€H™Öê?ëíÞ¦B½9?±ypõýÅê?¶:5êp]þ?«™#¬!9"3FGL J1628.2+7703@[×6&-@A(?º*3À:†±Ö§A"À<bf&¥†À‹@€MÃ,@Í¡²—ÂT@—Á_±@¿áàð|¬,¿ç`Çk¿åšãˆG"¿â3 C+ù®AGNbcu?ïƸ7¯‡^?'­±
uÄx?q¤•âDþP?xܕK7¨?eþœ‹î¦?k<ææôQ?ïÎg—›Ëª?yüÚêØ.H?cr/òƒú?g¾@gSj?n&8q°\c?s
tÀ‹­?îl
—8÷A?"RUEœ(?"荠ú…Í?ŒGƓ%ë?ž–wæ'þ?ˆ^Xß	?ïæð؄Í?kçò›Ã>ù­a{V?õÎiQêÊ?i­´e<=1?jðE×pЌ3FGL J1628.9-4852@tô	`0Â@¿Â±Ð ƒÀ8#ÙìpCÀ9ð¿UK?ø/L>h@ÝéÀ"š_?ùw/É~?ïù•‹–¢¿â3,}6¿ç…sq礿îA¼}Ê0:OTHERspp?QE|s©Á	?QKÜÿV?Î?؜·¶lU³?Ð
I´×¦ˆ?ã©fF?Ð
ó7'¨³?Apý«pyF?ZÇVq'?ÙO[	;#0?Ë`Aöa?ãSö;÷'J?Ëc^Ñ
"‡?––ùŒé1É?‰¬ˆî…ÿh?á
agùT?µ>¦Çú¥?܂]¤az:?µ$‡œ†Û?<irªõ ?0g4@%?Öy璑s?֜½Ë•9?äA(ë""?Ä8U=X€03FGL J1630.2+3733@NŸ C×Æ@E¥IÿþRÀ9´ s¨nIÀ;Ÿ0¡ˆ{d?úxuz*"|@©°Û.d?ôÅ›À?Þ,ôæØwâ¿Ü£9~Y׿àl³Ã¢'οïÿëÙ¾ˆøPSRPSR?–VÝï:=?šN~35|ð?êè»"%?È£¤—ØëÝ?ÄÍفU'?ÈÀª§fo,?§k"åÔÊH?°‰&/â?í+Ö5\w?¸Ï"L	?¥ÛŽ¶ÕnO?­4w?K•/?¸Œ
NœÖS?£oȾ鹚?é~^yóFÙ?­iýç`,?»áÈòê?¥ÀËOŒ?¿ÕBŠ7?±ó²2mh?éG™Œ÷£p?»j´?¶3!ÃZM?¯à"wÈ*3FGL J1630.6+8232@\ó(^ÃÚ¶@?@*@EjmÀ9<¿"ÀiÀ;¹½îãx
?ö*6ÊÂ[…@I¬3$E?þ9[-£&`¿ÒmOÄcq¿¿å¶3ƒ:2¿ä|1Ën™¿çÜŒ{›AGNrdg?çMjZµYi?ÄÜ{‡Ù?Æ£
¸k­?Àzr,Õôd?¸N—º<]\?ºk`Ýè½Z?ãȼTR?ËãÒ¨‹õ?Õ1Ld#ø¦?ÉA«±ÇÖw?²lˆŒÍŒ¨?²e-ØÄé?æÌß#ŽqR?²o²"ÝÃF?Ƚë­h¾?®+?QýA?¸0Ê1£ø?£À›¤þ©g?áSâï
ä™?»c§ÀçÀ?ÕÖ<åÐâö?»×=Î'Ó?¾ôðeOe?±£
ú=_¶3FGL J1630.7+5222@TÒÿ" @E2_×ÖìÀ9?¡F6E6À;'úÀûÞ2?àáøÆ®XK@'uiŽŽú?ÿæü9¢¿àí7[¿w¿Ú#{£¬\¿á¬ž=1'¯¿ß6"›¹ë…AGNbll?ïõÜe
Ê?KXuóûª?>Û®ÎW6Ï?:.Š'Ñ}?JR·A½?F'œ·¤?ï©V«å'g?'g´_³—û?wMê¬ó«?y'—\–÷Ï?tE\"¿Y^?uˆoçÙTº?ïOÐ1¶3?†]‡¢Lš?'L™˜€°?{JfíºÓ?‰¿ZsÚº(?~0M—½Æ?îï×çÕ)z?')>4µ[›?zpŽy¦Q¼?u6½Ja½h?›hßfñ<9?>¯ڔC3FGL J1630.8+1047@:uxmži@B/ÿ¢/À9›ÉØ)øÀ;†™°?ÎL?ár'3Ô÷F@éFÅâ!ô@o¬ÙO¿â"¬5[47¿íÕ=}µ¿â6}g߸7¿åÙEìüË¡AGNbcu?ïšñ:}?Nùg"œË?Z [1ü

?XÎ2:`Te?†9.qßs?,®¸
=?ïGš÷y¦?˜`í¨¿€œ?î@–:l?'BŽs"µr?‡Q˜õ!û?‰c޷ظˆ?íáéKÀÙ±?šÎÄÒ8ô?Ž…@~X¥Ø?|5ħ!ÛD?ª@$\;m?–½1Ó)È×?ëD\^H™³?¬"ÒUw? ã‡[Ñj†?˜É"caAV?½kY_Ò}#?ª%ŠKµà3FGL J1632.4-4820@uŸà·ö¿ÉA×ép-À8Bî'sÀ9æŸÐë??ø‹9L&õ@<öùñóù?ø5^ɹòÕ¿íù"ýW`?Óø/ª´ì¿åJ#ËÈQ#¿ê4zý2nPSRpsr?}÷#'l?‡›ø¬CË?͛׵ŽQ?Ë[ëÖÞ£?è]Öw·"?˽œ¹Ó<ü?«ŒðD0'Z?¿¦%:´Ÿ?Ó' ÚGÆ?Í:–¢åâ?䳧kOÓ÷?Ðd¹I'ž?°âø¯"vc?œí£›¨®Ï?ÖH$6{fþ?¶|5ª+?⿎Îѽ¶?µ"Æ.<n|?±fߖÝì?¯F·ûàÒ?Ø÷ÑâÝ(?Æ)?½¨äž?áW;ͽ/?ÈñA)¥3FGL J1633.0-4746e@uGñQç?¾ó@`å•hÀ6°\S½íÀ9aÓÚÞ?ç	÷¹EÃ@ì!´@â¯3+¦?¿§¾åi¿ãg´¯Ÿ•\¿ãvt€Û\³¿ã†.þE?ÐOTHERPWN?ŠXä»eÛL?ŽÕO:°‹Î?s´ÖHdÍ?†çÝì~æ?ïo2À'7Ê?–"6z?/?¯çÏçÛ?–©'.«?¥UC¥À?­"Ή£¼?ì¯Ù*;w&?Ä :¤R?·Ñ!ˆ?¦™â 5Ij?¬¼J§]?›ø£ÕwC?ëD1e–©?©Áã핚D?±Y^3X¤V?¯ÒÁ~d˨?'‹,3Ûd&?'1oç_ŠÛ?í@z×öV?±Yd	쁨3FGL J1635.2+3809@NŽ?é$@E+uÞÝqÀ6°"T"—À:¬Ò['@ä–ü±A@z®ž@©š¶$>Ï¿á\¿Uڗ¿æۋV`Ë¿çË,æÃ¿ë+ômáÁAGNFSRQ?ï£20Q.?ˆ êJ$ˆ?ƒèN.Éq"?ˆY}¦'?ZYx),?Y˜xºI>?ïÓ«T¨}ø?x9jý'ï›?eHÿ$G—À?m7³£ô©ê?g¬3:pd?mαu.×+?é
BM¯?±JЋ2ç?¼="µðš@?¦ÇŽ½—T?»XX?¢xQ?©£g0$?ïà®ÒI¡w?}þÉc³‹x?=ë­qÅè?pbb"!»ê?k"¸Pw?xÄí/®7í3FGL J1636.2-4709c@ubŸœèÙ?ÀèÏÀOÄlÀ7f×süPÀ9‡ëÕ¦"?ô"Þ+ÄÔÜ@4ýOü@·˜?§_Ö¿çñ¡B…a¿å©î{s>¿ç¢8¤Œ;ã¿èW}?pÙ1OTHERsppt?|K€ÕK‡Ð?Í'ÄÆ}?ÊMjEäa?Èr〠±Æ?é4|CïØ?ÈËÛ>ȏ,?†Yá¾nÌ3?Ž ÉêR?¼m˜)…:v?µEžÄî)§?ìås՝€?¶fëԞl?­ŸQ¤ÆJH?›Š:uö¡?ÕÅV–Âڇ?ºXШɗ¹?ãC_šR.?º}î
¬^°?¥÷1´àÇJ?§Ñå#ì¶ü?­
w†Òl?¡GVÛ¶ô?ìÏålDʄ?²:²–%7(3FGL J1636.2-4734@u{à~í¿ÄC€³CºÀ6ä'eîqbÀ9'!àÄÑ@=ÃòI´@ž>ïÔå?ûC¼˜L=?­Müƒ"À¿â8¶)ó'¿ãþÒ–³5¿ìö( ­9OTHERsnr@?6CâjOÔx?3D‰'!S?çBJCRBI?Ë­¥ÐEº?ÑuڀÀçy?Ë	ÖÎû¡µ?"~àJØp?>'{ÃA[?äWܵÃÖg?Ãí
u3/?×Mö¸v)Ö?Ãì¨y@?mêÇnêE?gÁþ
ú=m?é†{³0oç?´e+®‰?Énh𠄻?´5ð;"z?nÖ<[%ÍT?kø²Þ'wË?Þ{¾Á?ÀA's	1Ú?à£J¹y¦?ÀxP»•Ç3FGL J1636.7+2624@Fßß´0@D€C‡>À:FوœòÀ;Ú´*>—ë?áfà•'µ
@ñ‡î'ð@Pbà?êøì#eq¿âÅAµ?¿×-ɀ«Ñ¿ãÊ*î7¢üAGNbcu?ï´/ù¶¿_?‰®4ã&Ÿ?`ÝÎWÑNK?d7Þ
0:T?}yø·ªM?ˆ~0*òA0?îiÀôÅ ?¥§q{ý†ž? ÛGù—X?Ÿ¤Œü—?'¦IQt-J?"˜ÿ»¢)?îø%ß?ˆ¾T³^7¤?ŠYñå'%Ë?}/qŸ]'?"Ï¢jq:?~ø ›âo\?ë¼9 þ?®c+-Nž?§ûŠà.? Œ®€k?¶!™6ld?©×"‰»¡73FGL J1637.1+1314@=ÿ¥ßøù|@AÙÚÿ•võÀ:HNäi¡"À;›üD}Þ?ÇÇ9‹£@§ºu\M‰@Ä¿Àéz¿ì/죛"à¿è˜É:.Û¿ÃÐ'Ü}¿Ñħl¥ÎAGNbll?ïa›»?h2ÄF‹R—?5¥ºTc¢?;P»°4F*?]ON§Ã/?gõÒ¶?ï¦6b:ü?"¦ÚÝK?tÍT¨`bÐ?y*ÔØÔ?xz:"žO?y.ÁQ»w=?î×zE#Ž>?ÍÈÃÏ[r?…=u>1&?xýgùöÄ?šqü¼u¥8?ˆjY^íq?î¤NPÝ?˜¹Ï_Í?[¨@×[±'?m2EøÈ÷?¤Ý݄C"£?˜¤ƒº3FGL J1637.6-3449@u«•¿ðEx@ \îøœÀ9Qc"GÁÀ;"g¨…ŧ?ñWmû@
a–4à2?û¶¡>ÿo6¿ïÿ¿Ä.KK?ïÿ†ªBx¿ÛÓT"	•^¿Ò4>ñ'cÈAGNbcu?è~`ÿàj0?ĆJ¢Å?²˜')ˆ?«ö´xèù?ĺhk˜Éý?Áô½ª
?ëї9ƒò?ÃeáÎFäQ?ªðž5ûà?´bŸgû^?ºi$Bâ†?¼¡1«íµN?çÙï™?²¼õà2j?¹;öTyi?£+U©|rÄ?ÃúHw_Gd?¬úüùÎbu?æ1ÒC
?Ô³Á'y?Ì"ð"&ü?Âß¿S§O?·ˆfçïr?³×¤o/13FGL J1637.7+4715@RYÉ`0Â@@DñCÀI0ËÀ8'滋[éÀ;ž{Àj¾»?äôÛìû@~@T7$Y{œ@ð°ÿç¬L¿ã{·¨<8"¿åæÞP$R¿ä
këØο谨Ýaø÷AGNfsrq?ïöÉÈæ/?L*Úþ8i?;™ƒsÒ½u?4k¦Ù?G­õÞÑ?GA¼¶_XÎ?ïÔ;"f1-?v'²y}?d&`^µ?k͈*ô?g4U9·tß?l}?Ñ?ïgà¹]ÏÞ?€qzŽ•"?wYéÛGúŸ?nºpV<‰?ŠZܺèO?zxV­Rãµ?ïö®/å"p?]|òúSe.?	¥d9"?½rG¬s?QÖw9ÕU‹?]¨xé3FGL J1637.8+7325@Z~V>Ðö'@Aœé	:;À:è¢[ßú§À<<zØä2D¿¬'–°OÄ@ºðëeU?þ™é`+cÜ¿í]èK‹ø$¿¾­èlK¾Ö¿³a»Fg˜k¿çòג<rAGNbll?ï‹&þÇ+?• Kfã¥?‹Œx–
z?•o–‹ì?Jžn¤;¹§?IóÊ»L…?îýôvϪË?˜©©œU$?'øÿóyU?'ŽÝ_É0?ŠäJ.Z×?Œ2³ª'õá?í㷐²?¥Ô
ůúÊ?ª$
!Қ?¥Æ^¶á}Û?Ž'¿ˆî?~V•Ðœ0å?ï]´ÔòÉ?Ž¢ÏvF?y	B#"¶þ?|h˜y!?ŒW¸ùr]?‡N—)aX3FGL J1637.9+5719@U¨s¿ë<ú@D2Áð8À9ÎØuw{À;÷–uŸÀ

å@CsõÆN@p¸ßÚñ~¿êýiEÛ_¿æU¢å®×*¿ëñð¿åžo"r@AGNfsrq?ïû*¯ÎâQ?}‰±	™ì?çT5Ø?µT狥??ð»sßõà?}ƒ¦+#fð?ïÏä›eh?yÁ<}%‰Ì?cÝ}l®œ¦?j¬%ÍpØ?l=ç.7ü–?sv~†?´ì?ïoR…4#?+Ó¶Žp"?xÇÆ2¥ü?q¸üÛ7½I?‡ÇÑי¤?|—ïœÜLr?ïøëÃEx?Rìù™ça>óábýÀ?UK—Öpv?K¸lÒ-À?R´ìL%Nâ3FGL J1638.6-4654@uƀ"?u©`À7W=¼ùðòÀ9¥ýò߆
?þp뽨@g¹X%ÛÝ?ü·2Ü¡+3?Ç1i™÷k¿Ý÷áìåLjar¶¬¿ê*r.ñ…OTHERspp?s¹ë¨±N?uÔõ«¡Á?¸¶ž]cf?¿$
ãN{?ìÁ¸^6AÉ?¿ˆ¢‹.¯?{E–ÏZɚ?'$½ö߁?ÂU÷óJT?µ•'ß^k?ë3÷¤wØ?¶úhíu{Ü? #hšS3l?•$ˆ~'X?ЏÁvTïë?¹2kæf?æµè»0TÔ?º@ý¯Ì0?£¼WzæCU? øØ,?Ç¢–wœ©?±q|ôB¿E?èەs´¡?µ)ñB€M3FGL J1639.8+4125@PdzøÞ¤@DÎ3_¨ÝÀ: ¸jßrÀ;ÃiÔ¯ð?à›{'=™@"NAxÆ@UÀâcb¿ãõ×|B	ª¿æϐnw¬à¿è¦˜!ˆˆ¿ïýžIè½AGNfsrq?ï?[µ6ÚVµ?QuCìSCÍ?Q ¬£·r?NëïXúÏ?PZœ3Û?îüëQ˜.?¥'Ñý?¤®rä—*k?Ÿûj™p6?•£|̞¥n?"É uÕ<?ïP:ѳm\?'ûä	µlü?†ìÞÿ$!?wþr^XD?…é^´%"ä?v¿äæö}?êìiÝWZ?­D+Ùg¸?¹2¡#^£I?©îgÀ[Ž?®ÔãÍ¿?¡5nõÊO3FGL J1640.4-4634c@u$_•'Í¿"'‹Ÿ«¸rÀ8Ø{,ÇÀ9Ñ)‹ê"n¿ö0	£—Ê@
jthÏ?ý»¯ÞÕbó?ì} ⣣´¿â:Áœíáð¿âNªRNm¿Ô½p"ý°ðOTHERspp ?ˆ{òÃA?'Ý"Œò¥«?k'î$óV?yŒ{ˆÓ?Æ%d?–z´ï‰2?³"°kHó?¿XIä¤ÏÄ?—qªKi?˜ð|2vöþ?íóÜ¢4‡?À'ëã^ü¯?½"è¨1'¨?ªÖY7®i?«@H!]ï'?—z
aˆš?ê™~hãü?®žzÎJê?ÖñLå
«?Ë A±`˜??o
 7:??Lø'ìþd?äƒk¬0óÄ?ËĆ|0k3FGL J1640.6+3945@O¬Xߕ&m@D²•ÿ±%§À8æ…Ûv´À:"+,Ôta?øãW/ç¤?@6€´yS@5­ƒCl¿ÐbÜXŒ¿å~¯´ý¼ó¿ãÝtŽ-î¿êY©1<8AGNFSRQ?êÓ¹?â~µ?XR òqÐ?^èqŽÃ?…GLÃ!?ŽT˜›È`!?ïÇ`*.?}¢nó4±®?lz4†¼tÝ?rú)+?l%¡y%]|?q"Ae‹?æëQïu?´u´ýÛyÔ?¸@Cwéí?¥Ž³R÷»?ËÌ0üMca?²ãi'2{?îc5ýè*S?¤R嚽Ã?qÖq™QWí?Š­Ûþdë—?§'ÑîS/Õ?¢,u€®÷3FGL J1640.9+1142@<āŸ§Ð"@A–`)5ƒÀ:ÛeìÃãÀ;•ô©Š¨e¿âêz6Õn@Ív&wãç@]P¨¿äÌ®>0+¿æa†&(¿Ð­b…÷¿ëb$yµùAGNbcu?ï%«ÂÛ|ä?Ÿ®À¤¹ã?ƒçûï¥?ˆ'Îì[žˆ?'V‰­ØK?˜»<ˆâc?ï*™AŒúë?—•4æÎçg?ŒˆhpâŽ>?Œ©óì"ÞZ?ˆÑG+Þ¶Ø?ŒöȸÉd€?ìÄ."­?£°•‹VÚ¼?¦hW®d?–@¹‰MH?­TÆÃÂ?™Gîl›?íˆt£X$?¡—b'RÛ¡?sâP±ß?uÊVã8€È?²~5ãlä?¡
Å=3FGL J1641.1-4619c@u(; îÙ?®æ»Ÿù'À7'œh€òÚÀ9›œÈù¶¿ÏcôçH#/@
ešO±™@:_¢Qú¿åPŸŠtb¨¿ë%nâO¿Úÿf}›¿æ|Í{Hu»OTHERspp$?wü 7ƒdœ?–*-ûéäø?OÊÕƾ3?¡1**¦3?ïRȔ9Þ=?¦'óÛ!6?"u	ð©E?¥®àr¥—"?¦…ꉽ<1?±=&N…øE?íóùÞãÃ?µÃ6wF#?¿6 é£I?©A9¾i>?¿mHZÒ?ªq´`}Þ?è*‹'ß`<?²ÆLæ?»¬"AŒ?¾MÕQ®àx?f9{×ßò?jçF­]?ìt4x¼Ï?¾áøv9—3FGL J1641.8-0619@%¤rAeûÝ@9ÅYa›À8ÍÎ8׋À:æÃr°÷"ÀëýT©û@ˋo_^_@†î_ċ¶?ߟ'
ÈÊ£¿äeún#QÇ¿ãEk5œÞ·¿áÊÞ:ˆgAGNbll?ïž[³·ì?w›¤™È?W¦uÕ»?]fÇ[Ȳ?…tDWLº>?ŽÊ¬pcÏ?ïÀ~ÞíR?•¹n¼¡y?b¸z£	a?j`›|-ü?vdSê·Òa?"÷íòø¯?ëêÒ(»Õa?ª'—Úâ%?ž[ÓQæçR?''†'TI?¹y姛?§T1è"Jf?÷ûè?¡¤5RÝX?% K&b?M¸K{;?¤BpC™± ?¡Ž#8ÃÜl3FGL J1642.9+3950@OÀÍ_™Ã‹@DyvÀP½ˆÀ8"è1­!À:Á͐A+C¿ôÁ}ÿ	_û@;64D€8@"H?ß¾í¿å֜ƒÑ'È¿åÃT±¹Õ¿æ0'êðñ'¿æ‹Z˜
8´AGNFSRQ?ïíiæö>?ghy7W€?6äóJ˜ž?8Épýßä1?`÷¯¶¼¡?f"ÆpÚ?ï×Ý1ò£ë?v!˜a¡³ã?bêfL:?k÷%y']>?e8ÍøõÈs?j"ÕEpã$?î×
èƒ? fË]̆#?Ž!ÇHrGõ?ˆÖÅÎwcó?§‡ ½4åâ?œ6§'"b?ï¹÷K :Ö?}Ãñü<ïè?þ$ùSáÝ?°²ˆGÃ?n.ò÷öU?}ÀëŒö»3FGL J1643.6-0642@%"~e`­@8zE¿ý±qÀ9†ãOÆñÀ;…CÛ?™zVº@Ð@2*M±c»@'
 yó¿ìK1uT&.¿åw©Ò]'¿Ý|•DDº¿ÓÑýÀ¬ûCAGNbcu?ïªRÓf=?€;¿ßBz7?T–þ²† -?VyI	ï?;?y…é«Y6?~]œHÙ9ù?ïÂ0¨DŽ?|—g02á¥?gײ¢ÉÐW?kWùK"ØÆ?rûÞZxÐj?tfYד¶?íä/7™_? ñn#mdì?'è9Ð?™_±«.?¨½è>M1?š_2>'?íj«‰ðи?££¾3BÂ?N/¥*Ä??Rבš‹ÎJ?´nEu/$´?£ŒwªÝ]I3FGL J1645.2-5747@t£½ßÉÿ"À¨
`+8éÀ9–u—5À;Í#3᯿ör25J@
ÝeÌ7§@f+ —ºœ¿é7¤
zœ¿êäT®-${¿à.­i"¿ç^瘙ÙAGNbcu?ì}@Ԍá?½Øä«"?u0Ô¹ñ<?}ô ê(0Z?ºÂìùç?½dà/W?îCÇÑQà?¯eµï´¥"?xÓfwe°?…üAƒã°?¨©ÿr"?¬ZӖåË?ꐘÑP?­öR™S3??£ÈfpÚÒ	?"›ûEÃh?ÀˆT"m?¨ÉÀÒÏÖÓ?ëGîòYP?´¦ôJ÷?D€®Œñ…?I`ê8î?ÂËÈ
΃?´ #ãÍE"3FGL J1645.9-5420@tÏß֔ÍÀ'`óÀ9?‰i ­ŠÀ:æÂ:¢"=?î¨JG³3@Ȗœº
}@¸€nz\¿ÛŒ8óf"Š¿ìŠ!n«¿é3BL«ª=¿ïþNh†ÒOTHERspp?߆ûàÆ;?ÌZ‰—ˆ7?ˈ^eáÒ?Åk(kq˜?Ò´Ôì¯xÝ?ËꃤŽ??²ðh#Ûw?»T!µ"q×?ßÒ[bšû?ǵ¿*ñL?ÛqŠ"nDÅ?ÆÅr<1²ƒ?Ûe=ÅT™?³Úum½"?ÏY}`c?­ágÓ^x?Ôî4üM5?²Ò€¨kÜa?À|]×á–?¨µÂÌá:?ۄŽ>£'?À
ú¥`Ÿ?Ül3'pñ¶?¾x£×3FGL J1645.9+6336@W‹ž_Ñ÷¯@Bó©?ÿÊPÀ9ÑaE•5‡À<5ŽWF8¿íÍ2Ñhà@kC¡•f"@|/@_k ¿æö~b—µû¿éÆVv·Êæ¿æ_o¯:jµ¿ê'æ½õՖAGNfsrq?ïþÝæzh?,®<ol*Ü?°È'àO??ìšî#Q?$½Né@V?)ޗÉS77?ïË+%£|€?wì<žDäô?f¹ObN§?hx6WpÎ?n‹?!0ä?q—ˆ‹üã?ïXѳÿz?…KFZ©3?|ExE¾c?vQhôÑYd?‹¨ÖÝ_ۆ?4[ëQÀ?ïß\@W€D?oÀnó]e?0žñ‹–Ä‹?=ê1D2ß?náwàì?o8JÜ]Œá3FGL J1647.1-6438@tOÞ²gÇÀ(Þg@€ùÀ9»†ÜþsÀ;•BâL'ÀxwRœÚí@Þ
ô¸@ƒÄ`Á
¿Ü€Õ$V˜à¿å.ߥRƈ¿ã½Kõ÷¾h¿Ýÿ¦ù¬ÕAGNbcu?ïó€:ñU?T	;IÇ6«?£B"{ý¦?Sa›Cü™?W%UôY?Si$R³Ój?ïÇےùN—?~ÄÅ@²?Q`"3¯1ö?\¿Âõ;õ?wºvlè¶?z£ïºò¯?ï•;Ô?ƒŽ8m5 á?œº»óMå?qbCe#?"Q!¯^Þh?}ùqšÓr?ïå[¢_2?iGç}¨M>ÆT¿r\n>îrNÊĪ?jõ-Ä6—?iEÉis¼º3FGL J1647.4+4950@S)®_ú;›@DvŸ™ÛÀ8¢ßüTÀ;±m«Õ€?ëO§Á‹·?@<yX@nÈáÉ¿ä»ôbgÿ¿æüÓ¦8l¿æ"ÑËAæ¿äð滜‰õAGNbcu?ïò_‰RKœ?YÅ¡²ïðâ?F¨8ϰ ?Foº@\f?OÙ¡ç Ðd?S‡§Ym?ï'ü|?…ðd=F†D?|E÷£÷Ý?|:{‰å1ã?zªŠHd²?{ã\EÆ"?ï[ßmïŽþ?'	_Æۑ?zæ4Œb?oØ~˜â—x?‹ø1iÖ0Ì?Ï$jé"?îý°%?›´&¯»?'Ø0­n?zˆ|B?—W=ã	O*?™íOœ]sÒ3FGL J1648.3-4611@u6òä¼®¿é©Ùà(ÀÀ7ü¼b~À9íý©
ªã?ý#íãr֌@½•6Þcx?õ:7>/»"?ïò¦æ‰6u¿ÁIYvz¿ÞSªL^¿í‹9Ëím›PSRPSR?:dJ)"3?8j²â>Ƈ?ç[QþQO–?ÎÞ%QJK§?ÑBÂðÓ q?ÎÛÝL*gÇ?ÁO•ªI?69Bà?õË?ä(Vôfn?ÏCcæÔQM?×­×áØ?ÏC*ß%˜›?•IÞ¤ÍU?Œôýh¨°?âáà•CýS?º%a±e}?Øêú7¸"?¹àu:vÙq?~Í%¤•"?z?
L»œ?áÂí¬"øŸ?Ç/;ÇÃjÝ?ÛþðC¸s?ÇQí¾Œ3FGL J1648.5-4829@u-••ÀxNß·
CÀ8»
Z[–)À:m‰;}…?ΨÃ:VO@	R|N°@N wm?écØÏ[꯿î,™¥qØÏ¿ÓXå~
eÞ¿ã%ö 'AGNbcu?ÌéLߞ'T?ˆìꅿj?ƒ6yæüèQ?Š´œøeç?èxÒà|gÊ?Ì2o"ï{É?ÓúØ4j{?ҊåÁX.j?ªŒ´Ë®Ë?°8Çç¶o?äa²Ö?Ò(UÿåT?Ïݝµѱ?·a:J×â¶?³ÄºZÚþ-? Ì¡kNÅÚ?åG^ëÎ?¹9'Ǽq?׺û.¬<?ÂÚ½q8?q}Õ|ð%?sŒò3•'?ãú4XE°?Âsº7Añ3FGL J1649.4+5238@T}òÿf@CÃÙ?¡ÖÀ9'm;l¾À;ÙuxR!5?ïdí·ËUK@@¸Í'n@À@Že‰¿Õiïk¿áp&ÛèÛ¿å©
O…
¿ç½LþµyAGNbll?ï³%¡á?
ÙYÏW$?ˆ_JYæ@"?‹øïþ鲋?nÏ°ö…öÈ?x=>ˆ…?îŽ(f¨ ?¤íGË<I
?1'n¶B? ¡Nð»ÁK?'	rÕ›?@~B?î1ž?ÏÔø?˜Í1@u±ˆ?¡©±Âó+?'Ú祊²?—Êä¢zª?†¡I´šC?ì}Ė1Ĉ?¦|ÞSM¦?±‡7¦#t?›¤.dÜ?¥GPœÏP?ŸñPè¹<S3FGL J1650.2-5044@u.ŸðË°À«ÎÀAùõÀ7©ZÎyÀ:©6»}ïð?ÓÐӆi)ÿ@Ÿ,¾O¢@]'ßæÚë¿ä÷*JY¿æMc¡ÅÍ¿âÎÖ£vx¿ãZ/ðCۈAGNbcu?ïªñSY9S?ˆCi§ëž?cå¼CÅ	u?nî‡ýSµ?€J<Ài?"è)g'?îwc[Î?±"-'X9¶?wô‰Ü&?ˆä;¨ òÀ?¥žÁª'–?®Ë,Ù¦êè?é'áÖ-èü?±'ƀ|w?¨Tœ&:%³?šø	p‡–'?ãQ¹Ò¦?®uTºD?îÃâ4ž×$?–GÌÝÃ?1/ñ¨3V?6ÕVä¨r?£ŸžV/=_?–>Kì߉3FGL J1650.8+0830@:œò?Mé@>¢	Às"7À9lž#lÓÀ;nâO?ä~Oz!ëH@¢€Èè<@FÀ—ŠK¿åø~¡+H¿é§ÅËô<¿äIFɤ4Ž¿ïÿi¢¹†AGNfsrq?ïô‡ù
}?OV:‡½©?A	2jÏÅ?;ÕMíÏ?LÖéXû§?HkFt*õ?îèÞ©‹Y?£¦-þ  X?¤\ý½?œÚâYyý©?•P*/­¸?"@J0ù0P?ï L<£w†?‡vh¥õ›¶?‰—¼&Œ?€9CôŒqÏ?Šèg?eø?zˆ
[Ì,?êEQh'A5?¬RnËJ?³W¡_Kû?¢{m2€ÇH?º}Ó¯fª]?§¹½c\Ÿ•3FGL J1651.6+7219@Z³¿µ@AZ–`)5ƒÀ:ÌÄbšÿËÀ<$#wÔLô?Ö.u{N¢G@
êO²¥"?üÍ+4¾y¿ç5Œåj¿ÞR´úw뿳d™ûœÌˆ¿ÙÕ~5©É×AGNbll?ï¿Úýê¨l?‹2<ë?v/^\ÀRÐ?‡½ Ðcàé?cÆE[Öî?v3›1u.?ï­-J**G?€gƒV›?rÁ½Î_?p5'[¿Ð'?v§Ú}r?x!~zClh?îì•j	?"'ߢ8X¹?•©æV®èÏ?"ã
ɪ?‰†Óxì½?v¶ö
¼â?ï°#!3ë?~¬'†1?MÊV§c"?WX}¹#M?'—؏?|½C9âÿ^3FGL J1653.9+3945@OËôàM/@ClصýÀ6ÃðÈT˜À:(3Auì¿òBªפ—@ø|¨òþ?ûv'¿aª?¿×Ò9M¿ÜU,Ò,C¿ÒϰōÆÛ¿Ó%°)d8 AGNBLL?ï*ºdœ? Ô""Ví"?Gؾک)?P,–|¼ª?™éÿÆܗe? ¦œA˜$Á?ïÖ¬æÞo?x}Ù{¨u1?b)oâ°r?h¤øÿTÄ?gÀã7àÖ?qkelj"?ëR«åÀ‹?±K(í¬W?‰A^÷í?‹\ˆZV‰´?Âá?cU?°Ê@¤Ž?ø¨V?ˆif½F
E>Õ½õÁü'>ò†2ú~U"?Š
2;È?ˆhƒ9ù	3FGL J1656.0+2044@DDãõhÍ@A"'@	‹À9¿å¯ò¡sÀ;±b'¬K¿Å·zº9ñ@üZNU"œ@ñaÿÏX˜¿ãi Æxd¿è%/u5)¿á¬@ÒFøý¿å '<9ÁAGNbcu?ïö&êDZ‹?X$¸"h?!#ßA'[?!ŽŸ‹«øÏ?Q®ˆjÇ.?Vʲ㻚ê?ïÁ_MÊr^?|š?w¶?i×O)«a?kôàÅXÔc?rd±±ü9?t‰'šDÒ}?ïf½>®÷ã?}:Œ̽?sC;'Ìÿ?dŠQÂ!Ë*?Œ¯À² j?yú¿{\V?ï ¼¨Ó!i?|ðƒ»\?B: ¢u$?@FÓ	׫m?†­3É}~	?|kͱ
²Ü3FGL J1656.2-3303@uépÀ&Ì@`™?׆dÀ8Rys‡À:æ#wÔLô?sÒ­@³ožss@9·?œÎ¿çšç{¾¿éõÉß÷;¿ìŠ?£GÜý¿ïÿˆs¬uAGNfsrq?ïÄÀâ®_ž?†+w®0Òg?PUüêĤ?T;O<¿]›?yŠˆÕ-?…¾¤k&_?íUÌ'x`?´b1ûÔQ¯?'Ó<žüÂn?ƒÒÁV˜$–?²÷70]g?³'K»¥º?éüV˜À.?°Üwc¿?±Íñl•4É? r`£?ÂåïRdå?¬!´dð?ë'P{˜'?¯²ªñµÂÊ? åÆÃØJ?œºI̟Æb?»êŒ8ÁOJ?­"¿D™03FGL J1656.8-2010?ñŒlà@,%8@¹-´À97
ðôÊBÀ;/[àÑf?ô²Ãú@Mx@òûûcŽ?ÿ`%ßãí?ïÿ›BÞnW¿Û9'lIF¿àÿ£¿é׫»¸°êAGNbcu?Ȧ‹ÄÂë?ĝbô?ç)KQ):í?ȖÉâÇ@Š?µhî–¢Ä?»Û‹Ôâw?Õ¹âˆÜBœ?Ê·uy??Ü@¸TlƒP?Ç×\ù,?Ì
ÊEnt%?Ǭ€øòµ?ٌ]¶S°`?¾H¦
H«7?ݘ{Gúˆñ?½›ò¡"Æè?Á¶Nc_?§nTÌh­?ѱ$&HÑ?´Hsrü@?ÝYõ}úc?¾sÁ}ý´?Ðôæ[½
+?·À£sÒVÝ3FGL J1656.9+6008@VbøÌN"@Bµ²€l"À9Û²~líÀ<ÇC ¿Ð÷Q¼qq@'¹E†qõ@ûkŸ¶>@¿å eJT…¿è"²ÉF¿ç©ó_n᛿àßZYAGNfsrq?ïörÈ\Á?P*œ&H¸K?;d·s&
×?9·ŽÞjž?H…9$ùûH?J[ݍwY_?ï«°è
oÎ?'­ô0¢V×?r´wRaî€?s³[j™	?ws¦æ*?zZñ¼†?ïzî7j¢é?~Žç™Ž?u¡yQÃý?oæs8öð?†»¡h®cÜ?xd†…LÜý?,Öu¯?…fx`ô#ö?]/Å7ˆæu?]²1-F¯
?†qü#qw‡?"•œ¿fNŸ3FGL J1657.7+4807@R–»À5Ö@C>'ŸÐ€À8¥Þzt:dÀ;³r–'–?×Ü$÷ŽÊç@\z–9ý@ÍÖ©˜¿ä…ˆõ lÌ¿çEȊ"(¿æâ°ä0c¿âcóü«P•AGNfsrq?ïø³§1Š?H5þ\LT]?+Ŝä«DÒ?%ÚÞ/б?F?üV3?Eš]ùÃ
ª?ï՗4©ß?vž5‰ÅþÌ?b0hpÇ?g}"vL?h8ÆùæG?o‹¯
.?ït0ÜQ‰Û?†ÂÖ=Ø2?ræñNµKÖ?d*ð/Üý?‰€PDBã2?zÝ®'šØ?ïéåz$f?nGàÃ]oº? B)~¡>?'V½Ôôc?eÃõ°ž?mí&²¢Ü3FGL J1658.3+6149@VåT¿àU@@Bwìàh‹À:•€,
JÀ< œé°2b¿èl?Dþ%¤@¢A]îH@:»?†¨¦¿ê"Õ0.Ø¿ÜðÙ",¿ÛK€:;Õ¿Ö:µ-+AGNbll?ïæyí)ì?˜›¶þ?eÿìjƒ!?…•ÝÜÂ?<16´4Š«?@Ú•†Û`?ï¢öiO?†çȇªØK?vDP×_R?|/'5½P?x@z·Z?|ýJ¹PÑ|?ï#ú}?Ö!¬ÂA?ŽY½
ÕLu?×mÍH1¡?‰þùö¥4?r7Mßd'à?ï¹àñí ?vl']7?A³'mö­?FY\v©ª¡?€ž¬¥6V?u¸ýAëý3FGL J1658.4-5323@tíÏàGÓÔÀcð@uÀ8ž•Ï	½ïÀ:ðàŸèh4?þ-µÛC³@
¶tñ™‹?þó`Åg¨±¿à_Âáø"7¿á¥v»¿êù"iiü¿îÂi'¶ºMPSRPSR?^ïÚ©"¤?_ ïÜ
ñ?êSòËMñ?Çî"æ¤Q¢?ÆrUx¾÷?ÇÐØÔöo÷?P!nC?Xú›‡;b?ëIž[èôÆ?¿\°f•ˆ.?¹"xOê?¿PèŽ
Ã?®6~¤ÖÏH?›'Ô­7wÿ?èԅsÆì?²Þ±'FXî?Èc@û0|?±ÑT5m?€î–·|åø?uo5€ã?í/`
h?¦¡ÕjC?µØ²(¥#	?¥R˜âÛ3FGL J1659.4+2631@Gŝ¿™£@A¢¼ßï¿@À:Lyãñ¬€À;¾†ß'±÷?×ýißäùâ@ΔY=ÞÞ@­–@ž«§¿çeXøŸ¿äKÛyý‹Ë¿é³_
|…¸¿ØÙ,¸V~AGNfsrq?ïÈûNG3Ê?€‡—l é?rÑÙxç3?zI°*¸Èö?a`þǬhA?j
 1Ý<¶?ï‹3ru$—?'ª•íŠšæ?ïBöþX?Œø˜Ÿ U?{LW'v¶.?€þBÝ«™?î¥U¥Ýk¼?'úÊ»R'?˜¶,tUè?">вŸ¿Ù?š¼•Þ2|?‡¬×5›âÑ?îo8AW ?œé&M:Ož?Žƒ¶<xy?YÀæÓ38?¡kŽ_o´?—Â"¢3FGL J1659.7-3132@vØ¿p@¾$çùÀ9;\WìÀ:úszK ?ØY¬Þ^´@
<În7–@7ˆàcØm¿ãV<=%­í¿éÙÿÒL'S¿Ôš©ùQÿÁ¿ëR@¶˜GAGNbcu?Ç9à–	:}?Åسàw……?ü5
¢þ?£gnŒM?éA¦2E\I?ÇÁ¡}¾",?â׿;õ:?ÎB_~oþý?°¡Ç;¨xR?¬ÖK$1?×ÉÞ²÷v?ÌV»?¯‹?àÌ;ýå?¸þ^I>??¾8Ø}Ÿ·?¤0'š­x?ÖÙ´]hœG?¸¢Â)¢>¢?áäHñ¸€?¾Rý©sú6?Ÿ˜ÄOôð?š¤£éŽ9?Ûþ«)?ý?¾©>ß/³À3FGL J1700.1+6829@X⪀J@Aš¸GÀ7õKÏknÀ;2ƒ
?ñs¯g6@šÿ¬óéq@/EnÛ*¿ãúpø]¢¿åÓFœz'A¿æ`¢›æ¿ê2.™AGNfsrq?ïîL£:}?W·ÁMM×?XxqàÿÖ?T]ð–¶)?EܐøI—%?BXñMŠ?ïÔzÈ×	?wyHÁWW/?a¨—ëO÷?fl'+"G?iÝWKÙàë?pQÁPb?îþÝÓý)?'¼âE¤Å*?‰›­n?ˆ÷~:éd?5SàýÙ¹?…YŸJ†hø?ï÷i"…­A?]ž^VÚË?/Eʦ÷?.$ϕóe?P	ä¤(Ñ?])I@Ÿ3FGL J1701.2-3006@v{ 1ί@=ñÀL5äÀ8™'è|U¼À;§ú…l¼?üê·
ÈÀy@ÉþºÛˆ§?øDÓò0±¿Ô'\лnÖ¿àÕë/³L¿åÁáìï'¿éœ!3OTHERglc?'Ì®8o?wLƒcò?ãÃÞº¦?Ïèu)Š:?ØÓ­aËi.?Ð;^‹?°.E-7wo?¹¥"ývås?çMÓå#bj?ȡԖöD?ʱÔÖºŸ?ŏ.b?ËW8l·?v?±Ê©²¼êS?â!‡ÒW±m?·ÅP܆?Ì"¨IéúÕ?±:
ø[ž?³óÆ«f×D?¡ný/µïÇ?åç>—Š4-?ºR
62À?Îi"L#é?·þ…tbœ3FGL J1702.6+3116@J³Ÿÿå(
@Aá.ßç[ÄÀ:T'Íó=zÀ;Øèd?ð¼48Á½z@Ó/ Tk?öV‡¡ž&¿ëRHíã%‡?ïøvP`·ó?¿ØSË{‹^?·%ÂåËÔÞAGNbll?ïÄ· ˜ûi?ïù}ð®?r€nî¸G°?w@Å3Ty?fG‰"q?s#f—°?ï¥RÈX"Æ?‡}
"½2?wã#w¡öZ?'mC¬;…‡?usx\¦y?vø+ÀÎÚ?ê§Øæ1¡S?°`9$Ói?²éÖx‹=?¢œ€®åÓõ?·×bVnj.?¨÷ÛÀɐê?ïRõ¼Â#?•ú¶Ïóß?À¢êÅ
|?l†ãô2?‹bmlð¸?'çÎÏW3FGL J1703.6-6211@t'%¶™…À(Ü>úç'À7ðª4À;?úVôÙ?ìÔ:>a±î@…g;Mˆõ@È£Ìhú¿åE:‡:qk¿æU/ø¾¿å²Ê]ZÚ¿ìÒºû15AGNfsrq?ïáBÔ]¸n?dlaåC(?_å¸*=cý?])uM
;Š?]"ŸQÀF?U'¯*)?ï¸&±ý»?ƒ_"jOß?Y"íIK?`8؏=:?}¤:å.Ï ?ŸKkô)ô?í¬W­p¥?ŸÄ"ˆC7·? ÚJÕÆ<?'ëE^Å{Ú?¤[߯b¹?—:_–š"®?ï»õâ<¼Y?'NET+µo?=3çF»C?E#ÏjŸ6è?€è8V³e?''=b13FGL J1704.0+7646@[;ɟâÚ@@3S 8"¬À:gCÛ÷ãÀ<´SYCh¿ÙúhöRq@"cW=@—$ žE¦¿æedÿð ö¿çaÕN•S(¿æõ47?1n¿ïþëWýBAGNbcu?ïûþ
i?hÌøĘ¯?2ªQ?h¡ ¡´?*›'Û=Nö?59jËÜéŽ?ïÀº‰Xõ¾?|h%ÏòûZ?jqvFþ"ñ?k;‹o:>?rj0Ö±?uT¶a0¸5?ïƒñŠÐ?xTk3{?ÌãŒ=™C?p%n<bK±?~£#ä|þ·?n"êçû5#?ïÎèE£Ï?ta;uÀ·Â?O«²gÇ6?Uš]þHÓû?t–fó50Ñ?r˜«~F»3FGL J1705.5+7134@Y¿B¿˜0ä@@õ®Ú«³À:¶ïº€À< VrÓ\3¿÷ýò ï8Ý@ùÛQÊÍï@'¿_Ñ̼¿ç[¸b‡‰¢¿éeÈ­´¿¶x,rµæ=¿ïÿ"m¾RAGNbll?î£`¯×zf?³­è86ò»?¡!4æ֘"?±ÔÐØ£Ä%?'£nÇu?'P}­†w´?ï0eW¼Lh?¡j»Uz|ÿ?‹z€³Û©ó?"b—ð*¨?ˆl)];Æ?"—øƒ/O?ì,–ÓÎØ?¬òþ<"¯?²¹ÃÓ¤?©Ï"(bÅÓ?§Ã¤+ÉX?•—eËPÁs?ïeO"»eÎ?'ºß¯éŠ?U³ÉïxŠw?kÙ}´V?'úß	›½'?`2‰é'q3FGL J1709.6+4318@QŸÞW9@BƒÀ€æÀ7ÇÎÄô'7À;7[‹AB?ö(ƒFÆãÕ@b!LÖÈ@Z"tf"¿àóÛõ3É0¿ä³"›Çµû¿äÛÖS‰?¿éU*m¬AGNfsrq?ïçǽ½E1?c©u‡G?Z›!Õ#gÎ?ZÅöbM?UÕb°R7¥?Trǂ"¢²?ïÓÿªoå?z[=;µ?be*F?h.HVÃÔ?jå›RñË?rÉQãl?ïð«³?'ãY¾í<?ñ]w©ñ?‰?6öÐr?'x%B)E?ƒ«íÕ4RÂ?ïü­	-D]?Lçïº0	î>â<¬âu-º??¯{­v?:Ñ.Év?L»Ùk¾3FGL J1709.7-4429@uq"_ôöÀƒu€_¶ÊÀ4s 	ŠÃ=À9Œ";±†ö@
Êϓ%·@îô¿ÚöÜ?ô…¼/E½Ï¿Ñ3JøLt¿ß[o˜ÐW,¿äDb"4o¿ëž©<·ÁPSRPSR?,2Ú:Eÿø?54ƒEÀ	©?áBìæQ?Ò16"åo?ÝÈaÞêœ?Ò1÷Až?Qÿ]5]Î?Š]#_âú?ëÈòÎ_?̸¿]™û?ÃÌÝ}ŠW?̽®A¢©?D¤ä®Ëf?"X,~6{?æ|B´½¥þ?¸V>Óô9'?Ò}Uo_=©?·ò•(fë?䍚¡×Ý?;¸(že?î']ÏÊÈ?¦íëE‹ÀM?¦Ù ÿœ«?¦ì(¢¶tv3FGL J1711.5-5029@u&¸!ïÀã
é`À9W4Ïëe>À:ûy€žQ¿ì~Ì¿%@÷þ;¯®"@võ_"
Ž¿å2­[O¿¿í"š¿\æ¿å$˜ÎmG¿¾•`åHÈAGNbcu?æM8XýqY?ͱŽ˜å?g€Å‡ÜÀ¥?kW®ìß¾>?Ó6ÂõcÍ?Ͳ'ª
:?o%"á?¬D-h#â>?pöÚ/Âd?y}9è>\O?¥HÇ®~¨?ªKŽ~÷"¾?è-þ&!?µÌ{€é¤4?§p1RÈè?˜érô;É?Ê;²áI»?³¸E
]¯Q?R•î?˜7lº?ÉÒýh"?Ê!¦µU†?¥/8,`u?˜	Bp'à3FGL J1711.6+8846@^kYáó¥@;£Ó £ävÀ:p*ÜLœ'À;Ï(†1?âSb;+ª@
>àI+m?ù€@'&5¿î
rÓ©'?ÚtDìÍ¿ªmvûßßÏ¿ÇöÀÍK^	AGNbcu?ïïÔ1œ$›?bé0¹é?Oaa¼HÖ&?Qv °Ô]?P¦ëé'a?Xé'ÆÁ?ï¥j˜Ð'7?"íx\¤;?tÀF("Pî?zPpŽ]vž?xŠmoY¿?{-é*Š?ï9T[žs
?…!~Ç8 ?…'yïº[Z?8\ƒiEÈ?Œo(¨áù?w³¡Xö£?ïŠlk.¸þ?†kv"ÅI£?iE{K.ù`?q`µ™|õH?‡†a†
?"D¦doò3FGL J1712.6+2932@Iýöÿ¦=í@@ ƒ?»òÀ:D,_Ú[+À;›Ýj©Â?èàðÑlwU@Öa¤J"?ù4ŸWž¢?Õ-­zË?ï÷NÈKD¿ä¯ÀU"ÏÁ?Écu‡ãÛÿAGNbll?ïœ'#ú¥â?…ŠÑ€¤2?{iÒ3Ôñ?}nô"s65?v'›ÎØý…?z£ç–OL?ï›&bç'1?'&Ztþ«?zúiP\tŸ?ˆT$<¯i ?wre;ÚrÅ?'0}AU?-F³?™nÈgv«? lµÛ2ˆ?"/¸Ñõ¥¦?ž4ÝdNĨ?Š\òñ`J?í3ÅEJ'?¹¥<däúÊ?±Aê0ÜÏ[?¸ý@Nf¢?"®":~ª?–੺ÉE|3FGL J1713.5-3945e@uµ`ûH
¿ÞCë c¼'À7m÷¤ç«À9ڟ¹nK7?å…ø¼X¥!@
t×½ìŠ,?ùú¿˜†Ê?Ñ$†<oœñ¿åÅoá9k\¿ÐJ)"]È2¿¿þE?Ð$›OTHERSNR?ˆı¨Z?Á",'Çù?&ô€?Û?†h"7ˆ4B?ïaG.^?—?œJOE¶?'0!T"ö?¦ÆŒ-ø[>?"Ã""-.?ž
»ìk±¼?îÈeäNnç?­áÀ&¥ä¡?Ì槎;"þ?±¢†´bÝ#?­4xL	?›d>Úî?æ󗱨?²Ã¶sEÌ~?ÂnKª4?»NõÆ2+?r8'?…Ëî6ÐË?ë?üÿ9hÊ?»ÿqô"ß3FGL J1714.0+0748@<È%ŸÌ¹'@9/(Ÿ[zzÀ9cÇÚõ"|À;hèz0H?ùÐÄÔú@
ÕÑò¦{)?ûڀ׫Íú¿äþ̍¦‹¿ÖêDEÃóN¿àfr†ýr¿îÂÖF¯MPSRPSR?zBk§GTZ?€*ìlq)?îç;¨Ž"ª?£Xþè±³…?œ‡ð[•|?¡¹<íwÑÉ?¢³ùÍj?¨bW dÑ?íW Ï#.µ?³ˆ÷â©´?§Òêÿþ??ª´}%8·]?¼³µ¯rqq?©2Ù!¶ã?éR*dÌf?±nB×éù?¸·Ðýg+_?£/2,ºQ?½¬Ê-˜–?¯dÇÌj?èÎðHƒÉª?ºžå;¥I?»Ükñ´?­òV›gÞ3FGL J1714.1-2029@	µŸ´Á@%,ê¿üÚ²À9åRÒ4ëšÀ;;h7÷¾?ÙÅ¿'6{'@{6¢0—?õ€ïÿÕÙ¿ïÿñã?ïøËùo˜?Ù8'2"t?¯ÄõµE¾óAGNbcu?ïÇ`±ˆ¶C?¸"¿¢&?K>wçi!?J6g"/'ò?xçØ>·¾ƒ?'&l"ì?ï@Šòµ"ç? — ©Ï?pÁt·s
?ŠýÅTZ)?"¾`Ì-ƀ?mŒ&'?íJà2V,w?¡¼li¤W?™c¡}yÂ?'2êj1G?® ,à¯*?ž¼Õ`dd?/o
?"m4‡ ÎÖ?4FœÞZ?G]{ŽHiT?‹¶=L<?"`ÎûmP3FGL J1714.5-3832@uÆìà2Û?³´à
ŸÀ6‡à3±ÞÀ9©Þß)?úžÉ|5Z«@ìNµo¸õ@g(ñ:ë8¿Þ]›ç|¦¿â¥¯¢šÜ¿ã¾¬B鉜¿íÕÇGQÎOTHERsnr?gusâ7?cUŽwký?ÔR9.­_?Í"D´`é€?å¿Ûó5nw?Í8¿ý>þ?`)qNÉ?rºÔ¥ðè8?ÔÍ0:8GF?Ç×v÷
‹?å‰>qTË?Çö	ÙNwù?¥xA@'Ég?—í[‡gÆ?àXs†Ùˆ?µøK+V° ?ÝLFðáóÄ?´ÅE›KK?"×tÈÀ4?'rCÖ2×?ÏÅÜd?ºk#"I¯?çgÍ_x´º?¼H«Í¹[µ3FGL J1715.7+6837@Xә`#VF@@äå@a À9˜hô¶âÀ;Û k°R?õeڍ)ɨ@üÓТ?ý­ËOt1€?ÃØÑgç¿åý–Pía¿å(z‹LÇ¿ã
¯ÃžóAGNfsrq?ïé3p?o{úa6?Oûéºö?X3Äoöþ?^Ý*çõÀ?fŽKóó?ï¡X®;ì?"Á)s¿÷?vAÅæÇr?u8½õk²?yãšõP?'i¿=`?ëÇcíñMñ?ªù7M?±è8ÖF?¡1éåÒøÛ?¯¹¶¯çtf?¢$ûZP6æ?綾~"?˜s$Á@¾ø?"Ýœ¶)MF?ƒ@Íea¥?•|~µfã?•êâfy3FGL J1716.6-2812@vRÿÚ@S@ä%_µóÀ8ÃÆé]ýÀ:Íõ`iÍ#?ñMD¼rŒ@ÜJ)ÄÊu@ê@¿Ê¿â¬
µe§û¿è&Õ¢}þ¿ãÕíݾŒ˜¿ïÿò"²¢OTHERglc?ÔZ®òÆi0?ɇü—|	;?¿gj1'?¼æloO?áò™Y6?̲L+He?Òú¯ô]f?Èå9—6œ¡?Ñ®.é¸-ù?}/-Ç?ÛW!üSt ?È x³
'!?ÙE"|©$?´ó¶¯Ñ³Ë?ÎðÂëM?±~'9ȵƒ?×B데L?µ¾	—`b÷?ÐQø'¿o>?¯Í€›{^?ҁX4ãÖ?¶ÇP#BÛ¡?Ý,¯Y¬í?µêÏjR3FGL J1716.7-8112@s{ fèÀ7U* ½zIÀ:—íùm?À;Îú2`¥\À
ü¶!9¶…@
æÞÿ)k^@zñ –¸ê¿êÐ熿î'ß«¡¯?ès›s
"¼¿ç"!šYïAGNbcu?ïåH—b	 ?n"K¤ª¥¦?%‰»ß¥b~?)]–µ8óm?i^ÌßüA?mÎ 1Q4Ÿ?ïÊÆ«îS+?y¶.0­"o?NR·g!=Q?VÛB1"9Ú?vÒSòB	?v˜ŠÊú?îŽø3ºZB?ôÏhR&?"·ö1£?tj"H1à&?¢NÆÎô?Œ{/jæ?ïì\O¶z¨?qZ²†´Ã>a&^BŠ×>è;ÐÌ?c£Ÿ#'ß?qU|áÑ93FGL J1717.4-5157@u»`(^ÄÀ (g "I×À8›.­'tâÀ:îs#ä
×?íŸÃ'™þ¢@Í? §?@óNi¿áµh†•ö¿æqÃóà7¿æ6ö°RÄ¿ï1æáPãAGNfsrq?%gOù?£ÇrÜ`"t?lSNãå|?p.baÓèð?£>ìDœÂ?£]` ÿ7ý?ï.ú&›?¥¸H¢E@?my"£Œr›?yt?'èó?œ*îKIžp?£€@4;±'?èÊÑ"<ok?±²ƒF"z?­\œ[ÍÐ?›¼P-ƒ?Å}"`á?°u©Ð&?º0?Œ"î!D{?B?N‹h?SFo8?uğ˜»ë?‹–ù t03FGL J1717.6-5802@tÊ*Ÿ{ZêÀ'¦þÜêQÀ9KHÓ®hÀ;_	Ÿ»òŠ?u 5Ø
¥@÷¥LUC(@]€†£¿ä."Š]‰¿ä <Ð.Åտ䅄 |üo¿ïü¸#Œ:ûPSRpsr@?ë!wÛm?Á">¾³Ëý?§ª\Mø÷?ª¸ß¿V³X?»"^ Õš?½cICí»B?牃w
z?È÷$iù_N?¸ÃÍØ? 	?·ÏÖ¢Z£?Njó:?Ám\:c¿?ç<(tê?±i'ðë?Ãi¦',?¨ÁÏvÈõ?¿LŠ7[æ]?£"Åêî
?æ\ÆWP«¨?¶¸%P9?µ#¶Ø(_a?±D4ܝn?Ëû6©!¬?²µº<4á3FGL J1717.8-3342@v/€Uûµ@ވj1À7,ò³"À:(zúr!†?ðäH™w@ðU+%É@HkÀmmí¿å—Ì<%—Œ¿é3‹fŒ¿å¢`°ì¿ê½]¡¤^AGNbll?éDQLîN?ÇM'2ã?—DX»õ1?5ó+Ê?ÈÆ/´È"?ÆÙÑ)¡dH?ëȺÇßM½?Ç"É
eM?|D[éȳ†?ŒŠ}]iÝã?¿õäiå?Æ%÷,0æ?â"½å?´Â5ô¬¤©?ÀÊWÕº8i?©Šål26î?ӊö÷h?²žWùüØð?ëÕÉlø%'?²Ì‰VÅÏ#?dÌuœ']P?n¥
駓?ÀU¨u­ ?²¥
ù,9/3FGL J1718.0-3726@u۔€u?IJ¦ ÷­‡À7¾"Xð\À:I窞¥?Æá-;¼@
Òfhe@+äU¿çß'¶ÿ¿ãáäŒ3 ¿ß"ÂÇæ¿âœúÂSw OTHERsnr?™äid O?žxP	ïˆ?˜å6þkÎÚ?=¾ÇSËN?îiµ¼Á|ˆ?©Ïký/m?N9ùê:€?¡w!àÜ?¨¨Éäž*?«ALåƨ+?íó"ödI?²9Î~â~»?ºDFÇ+*Æ?¦lqé˜üû?º"Ãëî‡d?¦²N¯ŽäÓ?éfÞ©œÉº?²KsâÚç?Æxe‡…s?¾§Lçi‹?‡R âùõ'?¼Ôd›Ü?êœ'»d?¿y¡êÜ"3FGL J1718.1-3056@v0÷Ÿ©~@ !€ƒHÀ8É&رÝ]À:»_"K|?ä™fîC@ÂN™–@þŸßXë¿Ûi;9ßA;¿ëV¹"uÝ¿å#m\=²¿áTn‰ËpVAGNbcu?ÒHŽZüÃ?Çh&(å9˜?¯ŽLðê­r?²±)ë0‡?äâÔîVÈ?Ê É£ˆÉ?ç÷€´+v?ËQ{ îC4?Ÿf¿¼gŽ?£3	˜X€?Ì5?97Å4?ÈÐþ´÷$Ÿ?Ù9 ©ô¢È?¸k˺ßn?Ã\F<'^?«Æö
-âL?ݼLí	?¸ÔÌ]¥q?Ù¸áIõ?ºÉ)*ŠÐi?£óÉ¡"çS? "¡Ã0üa?áäRåè,'?»FGAá,3FGL J1718.1-3825@uÏÀ7"¿Ûe}`††À78CæߝŠÀ9¿6n@O@!w¤QX@î!è2-û?ÿ£NÏ?æl>;ÇMÔ¿âKW€–¿æ»\s¸"`¿ïIV^0ÎPSRPSR?b0$ŒjÌÿ?aN'ÝRå?Ù«üã?ÐàGªñ?ãѓ3?ÐàÔTY'?B&ï˜à¦?c$ÚxÊ?áÅ|Èöêñ?ÍÞMt3>?ÜlZš]¯?Íã'ü@9º?''Sq}(ú?‰$$´8,?àÒßEV{?¿tÔ]…?ç?Þ½å
]€y?¾ÅˆHxco?zõݳamu?vVöP§ƒ?àS¨ƒ !_?Ã5œ+¼Ë¥?Þìׁò7Œ?Ã?Ì»¹á"3FGL J1719.2+1744@CÂIàâi@<A_EàµÀ8Ãp@Ú»£À;L':ƒŽ¿è*"öØ[@³>\;-@WhÿóÀ­¿à;Ý
·£›¿à%–¯Yl¿àÿ[Ikž¿ÛÆ;IheAGNbll?ïýáÀÿŒ?*ª<º?}Æ4Ke9?%	bց?)¥ᚂ?&è´Ê'$s?ïÒX:3YS?|ò‰\Ÿ+?`c+5òo˜?f~í"×?mDš–´<Y?xù@
×??ïw}.Ì?~Æ®Ñ0 ?x]¯vJ?rè]¦î1?…ñèe'÷E?sç¸1Ž@?ïý—mÅ\}?7ü zO‰0>•‹Y0v²>ªj%{]?3?/ÅΘ?7úGNÇúœ3FGL J1719.3+1206@@ÜLŸëÃ2@9Ö4 ˜ü¼À9ð5³@3ÍÀ;~#yÌ?ÞüRF…@Q8!.£×@ŸŸ÷ג¿×r¯'¨ï¿åêà`ÓT{¿ÑŸ!='\¹¿Ø]0Ú_ÔÉAGNbcu?ﹿѬôÚ?|㳊?eßËÚr?gã£`òíb?x–'Cü%¦?vì{4
8ó?ï8'ˆy;ð?›-hL`G³?Š"¸ØŸø·?¦1Tê ?‡K¥	¼?'ŽÎ§wæ?îˆ$+Rþ?'zUàßç—?ŽegPAH=?€Þ;×H?ŸÍ'Òtü@?‹èƒ'õŠ?ë#;òXa?«'Jø7N×?Žqä*=?"ý©"c÷«?Á‹õE–-X?ª,;ð¢Zê3FGL J1722.7+6104@VŠÆŸ÷¬@AàP7PÀ9ó¡gÄ4xÀ;ŸáÝÖ
?ߑ±ÿÓ«@{7*ŽŸ@øýŸÓo~¿è‹t­¸¿êTÓSFŽ¿ë¤3Š\]¿ïþ™øRü@AGNfsrq?ïíy¸¨Ú?aÂu`w
¶?UtÚ¾ê1?[¨?i^	?O/h`BÒ?JÌ}^÷¤Ú?îR 2MUr?¢!˜Ïîã?Ÿ¯û╇­?–Vºcˆ'G?•ûýÓ¿Ê?–¶,§1í†?ïØ»Ö5P?‰«±ÄüÜU?`ÄçÍú
?Z4'<î?Ži"¤±¸?|8¦Kkà?èñ|ÁÀYF?´+¬ ES·?Á]³´2?±Ô\òÎl?¶O^‹ÅÍh?§ìí3̽3FGL J1722.7+1014@@m ‹]@8M@LzÀ8ˆéR>'5À;86%UúÞ¿æä¨Y·¶@˗I]A$@`Ÿ l1,¿ßýZ¸w+¿çÃÂÔj>Ò¿àqaûƒÕž¿áÓðÇË'©AGNfsrq?ïö웰þ?R¶jÐzðà?3ظÜ<?t÷Qh<)?Pƒ‹vW?RFHæc­?ïÏæ'é5?{»QØ?a8R­Í"?dÉSäX»{?ná*h³¨í?w}­0RpV?ï/DG§EŸ?ˆÂE"(Yç?wâ@XÆd?q'3mj?"V>{q?…ê–ftÛ?ï¿Íà?w½þ—B? ¬'è?ü›½ÙYˆ?ï
v—÷?w¸`.mh¬3FGL J1722.9-4529@uz!@W%À«"ÿٔ†À9ÍSÛIÀ:°;C¢ìÿ?ԋŽ®Ùò¥@
­ñœÆ@ÁeÖt¿ã@4}áb¿éÏ"¢¿³¿ÙwÜÛb½¿ïÿîbHÊtOTHERspp?º,±íNZ
?¿ôXQ1? " ñŽl?¨É©´?ë²'³DKØ?Âi#–; ?Û¦ê¶Ù™›?Î"çÙ5Bô?ÆŠSw?¼ñJL(ìq?ÙPPšªå?Çú¾®¸Õ´?Öx'$t‡^?¶F&QW"?Ƽ
uë˜g?«~5b¦Þú?Þ)Ó •¬n?·öÉ
õ?Ôwsΐ;I?ÁaÀsØ?¨Éé9a¢é?¤ž°c÷Ù?ä7§…!È-?ÂS{iø±3FGL J1723.5-5609@të¿çáüÀ&IFÿ˜ÑóÀ9ç**¾ðÀ;VB7²ô´?°_홃Ç@Lêik@ñ ÀTnl¿èæ¯æfÿ¿êò­Ï†}¿Î}$ƒmj¿ç×a"¯­WAGNbcu?ïƒÌYˆS?'+€ÞœŠ?ELåÝVÈ"?LP
l»?¸@$~Ë?'Ø'A3Ÿ?î|ÀMy¹?¯ÙÄÚÝc"?y€µŠ>?€ B·¨ûw?¥ä…="•?­{.r,p?íòD6‡&*?8'tm7?ŽIª°Ø…?€žVå`%È?©IQëW|!?˜á9ëN°?í#®]$?¨"ŠR—a?ZD€Êº?[œ¬¶Žà?¶Á}Yîà?§ò‹7ç3FGL J1723.7-7713@s»	 'RTÀ5˒€ ¤PÀ8ê̵O؅À;nÐ6䘛?í¢ز¼´@O·3ÞSÞ@ü?¶Ï5¿åQ¶†íοâù)Î'¿éØ8Уhr¿êú¹…$öAGNbcu?ï]­¥;?'	ìS¢"u?ºB<-W?±ˆsþŠ?m)Þ@yY'?pº®VP?ïwäPL•L?¦¸T}ç/?jUüÐhÚ ?kWÅb7
?‹ql¸ÀvŠ?Ž!õŒ‹¨¥?ì}m¸P¢ ?¥!wv&…®?±ŸLâ8փ? W,¼S–c?¤êŠ¶")?'¤'ß|Ã?î«âXÂÄ?—W©é,%?'›Þ™a?~Φ_әÔ? ¡ó|Wd?–Gêas‰3FGL J1723.9+4004@P8Z€¶–@@–ôÿñ½GÀ8ÕÁw.4ÇÀ;¨"Æ£½à?ó0ºø¹å"@¥³ŸTD@œÏÀr "¿äs°¢"¿å›{4îc¿çÂá_'
¿ïÿÇ/ß_AGNfsrq?ïå%·"•?i¨/G4G?b+Zw`\s?b‡e§([¥?Q^K¢ún?U%÷20ÙÐ?ï£sh0­=?†~fwÛá?vwHæk©³?x'N<¾Ð4?wÏ=·'?~œ||T›?íÑ#Üí0?ž6vH%ö?§vDÄ?˜BRÚK—ê?–îûB֗Ö?Œ¬»†+±"?ïye¼óìö?ŒØ±ug&?{«ÄjD.'?ƒÜœ±9?ƒÐ®â«?†øfî™&3FGL J1725.0+1152@A£_ëøâ@8|H 'ÁçÀ7ì=s(À:½ ùt˄?îJh[´×@…¬àa?þ*?›Ü?¿æë'Éý¿ÞÓÔmÕñd¿Õîqsp÷¿×e:´SP¬AGNbll?ïírí#j?g]—­Y?A‹ß4A?F¸3>d™?\T]ð»Fö?dÃ+‡o½Š?ïÎJ4|b?F$ôbÔZ?}ôóí—áP?¶-ÅÇÅ?ó|÷?‡®ÓžñI?í!)Æx¨?¥¡œâŽL[?™'K3é›?'öOìÖJ³?°'$e€i?¢ŽâZ¸•ç?éu[–CD?°ˆªMwI?…駳®ÔX?ˆÕûôV!½?Èclª?°1ÜR…Ð3FGL J1725.1-2832@v^"@lÚ@û6à÷IÀ8·N?(3üÀ:†–UAzõ?ó³'6{@;e[Ï_@Ìõ U p¿äÀ€æDm¿î¿'Þt†¿Ø+¸ëny¿¼Ç5oùbOTHERspp?åã÷Ëš?Ñ6©B©í ?ˆ8Ì5UKŸ?Ç_Éþq?ÓvJ'"p?Ñ;#ъh‡?ê—×f°??Î#ôÍ¿?µ/­2º?•ßp['ÐÎ?ąI"ºkÙ?Íu¬²R?Þ E"N«d?·´¤¹ºx–?ÁEU*CQ?¦©"Àtq?ؽׯ²ó?¶‹žLNØ?çZƒ¡
Š?÷\ZKÚ´?z-ïZ­Ð<?"-¶°!R'?ÐâBS-¬?ÃÁÁŽøa
3FGL J1725.3+5853@Ußϟåãõ@@ÿŠßÂr×À:cµ±þÀ;ïLñJZ—¿éù@ö#Ÿ†)@no?þȝ¿á ÁCà28¿à«¥Îö¿ä/vve¿ãñÍhAGNbll?ïÔƮAa?¦'Ïô{¬@?hŽÃ¢òÀ?•˜ª$\ý×?qî:×ÚÖ3?˜:5¢›?ïű:·Y?zïôC?¾?g¬Bñt?gC!ÀWv?q)AœZ»?uHÁ¬ix?ïhÀÔîð"?ƒ?‰‹H )?}á¡­ç,'?y.€c"È™?†ÞùíPH­?z-·¢Àƒ?ïÐ_ñHžŽ?st°Î
·?7j¤8¤+ô?;SôìiÂ?vY]&v@?s®
g3FGL J1727.1+4531@Q܇ Q»@@©÷¿¿žÀ8¢Ëlz|žÀ;¯ß´tç?õ`]æe$G@{bcL@¡\3\£Å¿äZÇ´Š
Û¿æƒÿíFâ¿émKŽ¿ïÿ{z
§AGNfsrq?ïêC\6ì?bñëÎ?_ç	–u?]?]x?G$}SgÊ?J—º$ªj?ïsé¡›,?'¿©Y'ä?'y¯ak?"ëZü|E¼?€†´éÓÊ?…Ã'"ª†‰?î…\˜]k?"¢–Êrø?Ÿ¸ŽŒ€½?'Jˆ'T?8žË¥#ê?ƒdŽÂ°kÙ?ïÞ÷݊G?šWõ'ø?'}ˆ_ƒ?'üÛ_g'?ŒA
Œ¯3?'{x_K˜ç3FGL J1728.0-4606@uy¬¿±[WÀ
€F6pÀ9:¬.Ǔ¨À:üº·÷R²?ÖQœˆj@
×i0EB)@x?V×þ¿éÀ	oëJ¿ß<Zú!™®¿àeýö:"`¿ìÁ°~ã_áOTHERspp?ÊɊé!-ó?Ä䫇ˆý2?á2I†z°?ͤt5ï?Ð6§Hs§?ÆáÏVÛI?âò(Om,?'øÂwp¦?Àª-ˆ0º?µþ%'»C³?ÓmëXJ?Å8§Õ£¬Â?߂}m*z9?¶n‹Ch¾©?Òoå/cˆŸ?µ:HÞÜ0?Ì:ÆãúP?°æ:œ»ËË?฽ÑÞ?¹¼;Ž‡¡?µÔﱞ…c?¢sMíoV?ÙIéö:ì?¹ûj'Úç43FGL J1728.0+1217@Anž i—s@7þγ#®À9u;â.]áÀ;= 8Ûê¿å´ñÙ÷'®@ï¼C͈@@w˜¿ÓNŸ~ú ´¿æ¬Ó;ë'^¿ã¦®Å¿é ›Žf_°AGNfsrq?ïêÞ&§t'?Œ¿TR%?J=k$·žÁ?TIÓYÚ¹?]$ý»\?‹3è7¢3Â?ïÉ( ‹ó&?{PG_d@8?f úÊmJ?iHŒø#Ï ?p[2TÏȗ?t/±ßZ°f?îiõÎÈ?–Š "	¤?"ÕԞ>­?Š^e•€'8?ëqŸvÀÅ?I$À%³Î?ïΩÿ?‰´êeÎ?@v™6k ?A­»ß"{?œ»ñaÇ:?a¼4±OE3FGL J1728.3+5013@SE@€"Ð@@ÃF߸aÜÀ9!EºtÀ;~JÏ1+¿ü=¯
@ìuN‹©A?ÿ[–~²­¿áÛ0–†ûÿâ*"Ô€Þ¿ÖmæÚ·i¿â$í|ÓAGNbll?ïí‡Ü"úè?c°5ä½ü?;øaþ¼Ã?8ȳ³D¼c?]òBŠ~"?aXëR¤Ÿ?ïÁŸÉ=n6?Ÿ7*ò¶?io~œÉP?oúDx?rx\ä=Ã?y­"7]?îâ®å£s?,Ñãê?…!:\óT)?xÙ|$ ö?™†"‡q?‰úS¨Àˆ³?ï'4¼Ù÷v?ˆyRJXn?©4žT9å?5Uòƒåˆ?9~`Ez-?ˆR
þý-Œ3FGL J1728.5+0428@;W¿PãG@4sÔ Ö¤½À8îdüÀ;Cí\M?òˆB+ž"U@Ɉ$Ì@ÀÿÿÕâ¿ä«ZÌ ÌÌ¿çÒ{•w ö¿é"i+üÄ¿ïúÊ;ÅJAGNfsrq?ï©ÕÑ9ž\?€:v¸ã5?y‰
±@?v~£mš…?q•ùÚ#!H?rXº`çe?ê¤{u•–?¹e˜d£Éã?¾B`/¬_Ÿ?²÷h+,Þ?©3ˆN½çj?«ãŠ—húa?ìå6BÞp?¥ç@ÓXR0?­
¹CÉø?Ÿqç—t/l?¤žâÏ?˜ ¤ˆ¤?á"™³µ5W?µÙ¬ë¦;m?Óë›Û·?¸ôÃ/c•C?Å;Áùs¼…?±Åde<Ä3FGL J1729.5-2824@vhË@p2˜@
!ç@–sÀ8ÛwˆÍ™{À:¬¦]¨R?üó…†QŒ@^köÝ@RtÈ©Òw¿ÊÃõùó¿êÄȼœÓá¿ìd1Xh¿ïþûB0&OTHERspp	?³«U‰`¼?³}Èu•?åÌXÔóÄw?Ì1›ç¹I<?Îøñ瀐?ÊD=Ÿ?¢‡JÝ]O?­¸0‰¦?árS–9?Ê_¿Ù/¾j?ÚÉö·='ã?ÉÀ™´'éL?¡_?åJ?¬•¨ÁEº?à7–Ÿ:9?µ¬ÿ˜f"?Ö?Ë3?˜è?¶:Ù`S`–?£Ÿˆ)°]"?–¬82"¹'?曊^?ÀòH՗T?ъ×晷'?¿)G3µ?ð3FGL J1730.5+0023@7ÄÊÿm3	@2-ß6[ÝÀ8Aðþ}=À;ÅJøK×?𭷀µG@×6aæÏØ@ƒ@7'´¿ßùnurý¿âh!š*¿âqõvlÌe¿æ'>×+KAGNfsrq?ïðŒ-X07?W¾é˸û¸?;TŠKÍ?3¨''C©?X'¼¼R`?VJÃýñCÂ?ïÀ‰Ö&?€]í'ë¨v?cí¹$«¿?fôÜh¤á†?vÞÞ?j"?zi'MÈÅ?îØȊïü~?d7Ó³5>?ŒXù.ªÆ?ƒE;BÚà?–ºqáiÏ?ˆAb+­Ë?ï–8ôš?† æTÒ[?A~5…€^Û?H"u¥Îå?‰ZâªÓ·?…µ¦5Ôµµ3FGL J1730.6+3711@Né"åx•@?\
ÿ7ƒ$À:p¨ß‡ºÀ;ÐaP?í±½k[@yò'>N@³À€8Iž?ëQႢ˜W¿å˜tÄ´5¸¿ÛIlΒþ(¿æüŋÃu¿AGNbll?﷓¯t¹Š?æ{՞U?mÉ^ôðµÀ?p%µëu?uQxË*à±?w-~9c?î)'îÕ	˜?¨tÏ¤?£>P*¤§M?¢z(¥L	®?"Q!Ð~d?˜ƒ_Èۋ?îh÷¬u%ü?˜.:̌[ˆ?˜CüÇ2Ws?J òñÑ.?š
ª(èÎ?Œ~Á¢]Ô?ëS"\`ë?³$¦>?°ÔHN7›?¥ '‰¨?¶ÐÓÎÁ?®RdFҒš3FGL J1731.8-3001@vW¼ ?ÿC^¿S À8~ŽŠqÞjÀ:…‡ú4ää?ðD%'_
'@
®>lL?ÿÅ*A*¿åf?²ûóß¿ÊKf»uâZ¿âD˜L׿á6g\IpÑAGNbll?׶ßg"%©?ÉÔü!¦ÈD?¨p&ÂÛœ?¤û`ÛÂc?❍àA<"?Ë#
	æ{5?Ü·Ýû¨?Ô0^3?²32'?³BGÊ¸?Þ»C1U€Ô?Ó`«Þ
ƒ
?ԞET×Ó?¹—]0—?½&ÜÝ]?¥á°®³8ˆ?â
¯¹ðk?ºâ‡"'+?Úó³»Ç'{?½ïŒÐ4?¶8dÙ"?¬…_"oÎ¥?ß~3
óý_?½±¼•|È3FGL J1732.5-3130@vDüÀz®ó?ð?8?®ŠÀ6 ?û˜'3À:3X–š@
u9ó–»@FÿÙ> $?ëÊS0‡9ù?ïÿ(#,!¿ÂwÕRò.¿äƒÊ'´'‡¿î3&‹ÉPSRPSR?³.·ÿU¨?šÝzŒÁx¶?ê¹
о?ËùÉ샓­?Ä"Ý=Ÿ?Ëg2‰M9?ZðJÂ6¨¢?ˆe¶CìD?ë"±a…\?ÊK&ô}?Ã?Yäg<?ÊĈ÷8Á?£º)|µw?š…µ´8?äÖZ:?¹~$N0éÞ?Õc'.Nß?¹
va6:Ê?;×Ëî5ú'?@õNS;~?ï"WŒ…?`'»Åž?ŸlUÞ¶wè?éb/… 3FGL J1732.5-5048@u@i³únÀ"ÖÃà'TÀ9}:í;ØÀ;W
V›H?ÔÂS*ä@$QËú"Ü@Fk€V§'¿è¹?H·¡¿Ýqtºf³¿èú4È«ø¿ìê×ýêPSRPSR?èá+ãUÔ?Áa"%I¢Í?ÆrÌś}?ÀXí'ú…´?¨%>"4Æ?§Cʸ ͧ?é»Ý¤˜+?āã£êëá?¡UëÎä·?¢ïˈ¸µ?Ä»yæqŒ?Á©®ÖýH?èÖe$ž¬?°øC|œÀ?Ãæeúµ÷?«:_QÛ?³!
Ež¯?šó¬?L}™?é‡LgtØ?¨¦\T!BÒ?®Ù{G‹?ž°–?Â-|ïg;?¥V$Õ@«Û3FGL J1733.0-1305@(÷ÞÉN"@% 6^`ÞgÀ7'ÎuCxüÀ:¸M`Ûâê?õ5ÁB€D@Ç2]Ë7K@éð»>"ö¿ân¿«œë¿æ'Åeòš‰¿ä­cÐß׿è*»¾—ˆAGNFSRQ?ïÀ"ž8š>?€å}²³â?W"åþK©õ?SÕ]²ÝÂ?yíwdöí?€_3Xdöè?ïh'vq=ª?œIø[»Ø?eNÁÇæ?n®ݘ>™?CÙ8Å?š‹èíçx¢?í¥×ܼ¬ó?£	@YuFú?•÷pDÇÍ`?•Ë¦š?ª¦ÊÑJ?ÄÐxÔ?ïåå[>?q+ëÈÑ`?–`Êâ4Z? ÿöòŽ
•?iÈ¡!º8c?q'ðÍ»Ü3FGL J1734.3+3858@P"ÿÖåU@?…_Oñ°À8GuÇ,yÜÀ;m>m#
?ï6¨ê¼@]®:æ[@€…Zmà¿áj0]Égp¿å­è…ù¡¿ãÁ5,»''¿ë_š‰ŽAGNfsrq?ïïǚËÀm?UI¼ÓÝsÄ?Rîó¹Â?NÍæ&gU3?K­]z"ý?F÷°ÈË?ïÒxa¬'?xÉɱ¼hs?c2´Ä®]
?hGüӎþ»?jMÒÙ¥×?qíµÜ$™G?îŸNYì³=?•ÍalÕÈ?–ò˜¦Î¼?ŒƒØâ÷¥?•#œ¦ÂɆ?‡£ž"Ìg¬?ïóú‰ï"?cëþ:ü?é
'l›?1¤ñCÇF)?VÜ[x,b?c¡Ú†3FGL J1735.4-1118@+Æ!à$˜f@&sA¿½ð'À9OsGö8×À;4žm>¿êšŽÇ-¦@ç\20@@O¿Û͜¿Ððs{ÞÙÑ¿ëºeð°èҿΤf/0¿ØøáÎ;·¼AGNbcu?é	`Šh?ȵ=Q—Z?[Y@\ ˜?[JrÖUÐx?Ë¥/üÖÒ#?Ȧ¨†YS8?îÂ>š"ô°?§™ç¬»"?l²VŸ£S?ri¶=ìÎ?¢ðí¶"
?¦Vg³z?é=Åý°s?´xl¨ìñ?¢>OU'ö?"RӞÍûÊ?ÆyTG7ô8?³|©/åS?í‹Ó(FÒØ?¡'oË6SÜ? ]D0Ó?"Pæºnë?³š>¦xhö?¡&
=êÔÇ3FGL J1736.0+2033@F@L j@9k>¿XpÀ9rêUrùÀ;P…Ûv³¼?ð%ä‹Zf©@sòoɑ"?ûŒ@ Y&b?ïþI™HˆQ?à6¦,Wª¿Ø^~ŽXüN¿×–fUÁÊÞAGNbcu?ïÕ3ìRd?uݯŒ–w¸?l·;Ƨ÷K?i¬Â5F
b?\+NšKë?ob¤MZ]?ïAÈìÂï±?ž@8ºw¿?‰¤1~6mÓ?­¬ìøK?…é"Q
¥´?'ºé¹p3?íN5ü¶Á?¢¹t}ª#?¥pǚ#±ã?—h`‡®zñ?¥®…áÿ?šÄu׀G?ìrTo!ˆÈ?°×œŽ<1?­ÐeZ‡÷½?¨Á/ل'?«
S³_{Á?¥'ˆ½Òç.3FGL J1736.2-4444@u˜¨ÙºÀïLßזÀ8ZHùn‡À;S‹'?ó1£™D_@ˑô^·@'`gÁ¿å±öy|Ä¿àÀЪ§Þ׿æMÞzt:d¿ï#û½{ 2OTHERglc?'…½Ž5òù?'<G´ãè‹?íí`"p-Å?´›ñ"ή¸?¨gñâ*7?²9-füŸ?…F$º«È?'dÇ
î?è5º—z?Âåùª½Ãà?ÍÔ³Vm/7?§YEb{S?Ι|'}«?°µQ'~¬"?áô¥–sÙ?¶wşÕíÓ?Ê!Ò!²î?­pGK6?¸·3\áß?¦¤‰"?æ¡z–0e?½—vËí³?É g6°}?µì"E¾áÃ3FGL J1736.4+0634@>EÑ q$0@3¤:?–îÄÀ9 QJuoÀ;G›	b@?í10âKF@êßp"eù@فà?pX¿è'%xyR@¿é
ÎM$¿è@doÒ\¿ïþ÷‰[U^AGNfsrq?ïù…öjº?C:¶§]c8?;+‰7?6¥­Z•?8¥D%ã)ú?7§•!Àko?î‡üô¾?¢õ=¢º?š}æà(fª?"ÐNƒ0 	?"'z_×Q?šñ³©sÄ?2ô˜6?•
ÍV~L?™Â"a\Þ­?{­!%d?"ËÕ@™?‡µÓ`7ô?èÌr0u?®Ã×ô?¹¶²½.›—?¦¡ÊhìV?¿èôw?à¾?ªØÊe9µ3FGL J1737.3-3214c@vD*Ÿ{Zê¿Ï*À1äÀ8kógkI$À:|Oø?óÁwO>'@'ˆíNø@$H¿aL¿È4ì›Ê u¿è6U'Ìc¿áȵ¥8¿æÕožŒÙOTHERspp$?t›ênEY?vÝÐËYÃí?ðËþT‡?'N}Í}1?ï_û+'#?•Ê:É?˜ˆoŽ½?©T~ÎoWO?²Æ±é9?¯Œ³Mª1?ì낦JOâ?µÕ¸ª}?µs‹czù‡?£›)]Ta2?»èB;ÄI>?¥Û1ò.|?éԆL§?¯B]ò݈?Ŏ?‡°|?ºñðžmh?¢]aM}K?›pÄã&±?évš	bÃÌ?¼>Sg=GÒ3FGL J1739.0+8716@^Þ˜¯@;ñ¢@1HwÀ9§~b®–À;Ýî­È$Ç¿óÅΞ^$y@r6xâêÆ@7ø¿Äс¿ÔcÏÁ&"¿çÕ¬A3sl¿Ü
û˜/ë¿åŽ¨ê¢ÿAGNbcu?ïü«Õ¡±¨?AI¾"Ä?Vÿ"'?¨Çò':F?5˓,jÖ²?@
©	­çô?ïÓ(«ONk?zŸD*¤:–?^œSG¼º´?cCm'!Úb?m‰+Ó7X?v'ArRÕo?ï@WG̟?‡0aVи?º©<v9?zEžUÚ7?rgèÝ}?'z&¶€(°?ïý¢ÙYž?:¼Ù{`W>¡Œ°±'G>µU€—ø£W?2ànÙyQ?:¹îŠË@µ3FGL J1739.4+4955@S8ß¿î—ù@?¹´VÝ\À8à±é·ìÀ;¨Üôb=¿½EÄh@9¿ím@tÔÿ÷«¿ã68š6ˆ¹¿ãG×æÂ}z¿èÈ¿%璘¿Û¢'ĹAGNfsrq?ïô°Ð·0?WšzŽ?Eó5#Jô?L/Bjkæâ?GI‡þ¹òµ?KîȦ*@
?ïÔáBj4?yYZ E?`0ü1J«~?g2ÖŔ?jíÁd?«?t}t6-Y?ï?°˜>Ÿ?‡*¶º™Iß?µ<ô€ô?xk@BþUš?Ž^œû×D`?Ë/m™"–?ïü!±W3?I.©¨'àL>ÓtnT‰šH>ãÙ[Þå?>©€»ô?)?IØ'$Ä3FGL J1740.3+5211@Sム3Ï@?Ê.Íû¡À8|6™AÀ;¢¡€è?íú9wEï@Úæ1ø @ž¿\V˜¿â@þŽ`¿ç%ÇçØ
j¿é¥Oê<ãû¿ßÃì]$¸
AGNfsrq?ïö6l
#?L™Ñ{Þ?I ouÙ¤?D¾'ãÂ	q?;M"À«8>?="ìºÎƒØ?ïÓêw/k?x'ì¸Ò?ba[€Ô?hÃv«0•Â?i´'‡OÀo?q㖒iÂd?ï@ܯi`?†8HÖýî?€dQ"×w?wä²Ö±?d' Ð‡Õ?QÉôÍ«:?ïø'TzS?Z(úìþÄ>ø¿Ñ??	ðTY'$x?Lô¶ÿŒ¿Õ?Z

¨¦z3FGL J1740.3+4736@RÀ'¢Ü@?SÂÀ®À:gø[ÆÐ4À;ìP->ýl¿ðÑÝgú*@攸‰Hé?ÿ&Šþøï?çâQ]¸q¿Ù£»vc3¬¿ÛúS0‡9ù¿ßþ«íŸðAGNfsrq?ïú4>?FÓ¿Ìu!?8ɏMâ–Å?@ï¶S<ù?5–8(-pF?4ç0‡¤¹?ïÅ>F0íÜ?}sÔ}Ì?gìñ€"GÞ?jó‰Ñè?qjd'>í6?v O""T?ïKèî?'-w"R??"Ôô®Óžì?x!õã"?Ø?ˆeJ‹r%?s¹¥\X«­?ï°[ÄïP?~‰	>þG?3>G¤Ò??6ÇôîÕ?ƒOI߅]?~,£Ec33FGL J1740.4+5347@T[O?Ù3ã@?ã$H¸À:h\ïÅYÀ;÷Ÿ<pÊ¿ç¾W¢:@
ƍ³\cX@&"_ ¤{¿ì¶ø–‡™¿ÝKH·Ì,¿Ðú&2ë.¿àÎ[‹Ó§AGNbcu?ïû:
?>O¬q(§ª?2}¹8ã×?1¨7ÿÉT8?4‰\ö´åN?4ć_ùˆ¡?￙MÔ1ß?{+=¦Þ\>?k®øJÔÊ×?l¸›|Ï?r[Üð|«?sQÙ=o5?ïT½ÕÂj ?€î;	ur?«×«€ú€?t]ZÓ®Ï?Šúž¹¤û?v—#säŸú?ï¼ð—F°?w{%—$O?1£ê'B¶?;}¹$g•)?€6ºêœ>(?v¢ð³:LJ3FGL J1741.1-3053@v]:à;>š¿ÊUNÀFExÀ7â¸ø²<À:Ò³–šâ@Kڞòt@ý¸§ü´?ôdÐvû_?ä-v€dê:¿ÝW¯¿JÙ¿å–œ>‡È¿ît>ág8žOTHERsnr?Yï½ª?^®ˆ'úۂ?ߍ'Fôá?ÒÎ3ý‰Ä?à,ïîdõ±?Òû–Ô­N?PžF¤bv?n$à/á^ª?Ðrʍ'Ã\?Ɔƒø«+é?ç¾K•äí
?ƌ…µÉ`?šgÇV6b?".ü=Å?䏄d'I?¼EÃ6­¬3?Õ:†Êf	_?»umàøè?£Ÿ‡*ˆ=?šµ*!;¦¸?Ø¿ù³U?Ä
Ò7³År?âoº}Ò?Īï–#3FGL J1741.5+1351@Bð¾@Bo@5¢Àu¦uÀ9äêÅX/À;'H¸?ñÁ˜H¶¨@"—G…@Í,@zÄl?êÕû]·t¿Ü6]`¤0¿æþ5¹['¿ê
.Ž€-YPSRPSR?ՂÿdŒ%æ?ËÍ nd†?ãŸÕ6Ë}?̊øÞåJ]?©÷—ˆ2?­XÊ ½&?ç¤P[	¼?ÇJ‡ËÔ#?ɹ1€‹Àî?Ã`¥ É!R?®Ùdø `?°v¨R¤R?ã%X˜šUš?½âØÒ)?Òh[€tÏP?¹÷ÒàH?½3Í9Zé?£(h©¿s'?ÖÃ¥·àÎo?½éô¡âò?à"S"e+?ÀäˁÕk¬?À(«C´Ît?³ DÈ3FGL J1741.9-2539@ÚÜ QÚ@XÀŸ—à\À8µlC9À:m}F|¼¿¥²ŽÙ³KX@
ש`Œß@¥@¿ ?é>ˆÅ{¿à0àÍàž¿çÖësd¿Õ¸ÁÀ»AGNbcu?³šBz£\?¹†@ëS"(?µ=
%+.ž?¹Ñ˃`j?êä«EÁ?Äat$ʲ?ã²I
m{?ÓÛíÐÒ?›ÇÔÊä7?¢l<øtñÌ?ÖÞðªpvÇ?Ó8¸»y?Ò«=é¢?´´Žë2›Ú?¿‰²§p~?¤iñ'R`?âÊOÕ!
?¶[!²]ìR?ÙC+fvÒ?Ão¦ªfB?­Òâ
é?´ÔW±4?âß²öý<_?Ã+µü©3FGL J1741.9-2054@¨u€4ì@˜ F†øÀ6Û¸KgÝÀ:˜ùN59@	ÈWQölÙ@°5<wÕ?ü&µü¦¯,¿Ñ½Zý/HË¿ã:*k¹b¿í2äÝÿhð¿ïwÅiÆPSRPSR?V'°±•æ6?ocÞ!Yg?îŸ.)»Ý‹?°fñŸ})?¥X‡Þµx.?°<° n}?-Vãš
~?DHÃÀc÷?íº˜Úy?ÁnBç/g?·ÓÍü&ç?Á؜Vã?ˆÕ&ݺ¹?†7­;…R"?êg˜f6SQ?¯–úw5?ÄàѸ×?¯\Õ6¥Ý/?Eøbj¿?t"¼-?ﻌ¯¼˜g?|lW÷Ó?€ìH ê?|:߬dT3FGL J1742.2+5947@V àè@?Ï¡àø0À9õ@UZ¥hÀ;ë½¼Ž'(¿Ç®ö£
@ÕáWHfK@hÆÿ®K'¿êН<¿ämtkH¾¿Ütû'毿áZ3RÆTAGNbll?ïû;9;"=?AÉvûÞ
Ä?%ÚBîæ{??%ÉGLJE7?;9¯zÌÔ?>ïÝ
ÀÐÊ?ïÇ^ñ~Fã?y'¾@ÚÜ ?hC_Ž€?j
ÙÄs?p/3,Çç?q¦%fÓÖb?ï'q£–…?"®?i€A?vtCÌlH?yXú£E‡é?")u4(–¹?xåöõ·¡®?ïÃ8Ía*?wl(—5D?7Ò´Q_h?8¿+¯—÷?|æÈT9tÊ?vúµ|ñÎ3FGL J1743.9+1934@EêG@0q¸@7Wà0VàÀ9ŽÊƒ*ÂÀ;Z´Î©Eß?ÜýÐö…¶@
(w¹õڍ?ünJ 	µ¶¿à'󆹱׿ÐláÈ¿]¿ÍíÖèY›'¿á"'¶®"AGNbll?×ѐ?ˆwä͘-?uay)n?v6h"Ø?~œ³wžŠ?'ÂoFTõ¥?ï)€™Í?—Ùâÿ*¡¥?‹vzi|?…ÿµ!ð£?Š)ÚÚV—?'Žœëcb?íÈÛ>†Õž?št|§ƒÕ?—Þ>úˆ—W?ˆöõ0;ì?§ƒ,šNZˆ?•G)%ô
/?ë÷Xy*0æ?©´¸˜T?'*›­?‹Á'?¤?»ú¹OÃ2'?¨ž
Dòq3FGL J1744.3-0353@5"?·¥ô@*
N wmÀ9œ}¬ðÀ;ŸÑß[¿Éw"\‡{›@
>µÿUá@'WÀ0\>?å#Û´ÇŠ¿åcÊøÒæ¿â݇®úBÁ¿æJ~É0õAGNfsrq?çás1÷˜µ?É"™Öÿ?ª;ë^ø~?«ðùôQØ?Éë8`c˜P?ÇGFafŸ?í þƒÉz?³€aê¾±b?7€‹J¶?Ñ*"Ñ?­â¯Ò
f?±D6ż'Ï?éÓێy!h?¯S{N¶±y?«3®qË?–ÏÄýò~Ô?ÁãÑ›?«i×úrA>?äüHTT$?ºOP.ç ?˜8+¿í?xäf0c¤?Ԅ|³X~ç?º#)yÐnþ3FGL J1744.5-1133@-¦C?ñC@"^C ÚxÀ7ö›ÅÃÄÀ:Ùxà¼mÚ@.Ħ7¸@Øâ'q	@'¨ëF4˜¿ÙÉñÛÏôõ¿àÚz5Œe¿ê£Ö0Ωò¿ìÀ"•W¿PSRPSR?\´Dd`Zø?^w8b0er?ï"!%"0?'abe9?‡¦¯*èÎ?SB¥Å…C?kÌù—d×;?x­0MOº?íË.
—'?±m6êä×?°È'ƌij?°¯Ý;Ѽ|? ña'…¹?"ýM—Aú?ë¤ÙX§4?§˜'ó݉?º`†»ø@?¤ÚQ¸?z¦±z…ßã?r¾i¸AÄ?î2T<\f?¡›»Ï©M?«øŒé}­? Žx"¥†3FGL J1744.9-1725@#×Àâ¯@^á¿Î¼À8Å]Ó6À:ä9]ßË¿³»ëñ-¾Ð@9òj@›Ä?àj¹¿éùrû¨µõ¿á
ąšM
¿âÛ¼…¿×yµAڄµAGNbcu?î&Uj€®?°cŸÈ0?q¬LâT?lç¢Q?«bSÎXÚº?¯†fì8©˜?îL¤ªè?®bƒîÜ?uL`ØÊ­?xÒNU?¬o²¸??¬æÌñU‡¿?éDÐ2c?³‰½Æ@·??©¶ªOmv[?™¦R ː3?Å%B+»ØÝ?°e­Â?ëbY!êü?©Â¯T?ci~ہó?eeOĺ8?Â(÷*X¡ß?©¡†‹n)3FGL J1745.1-3011@vmú WŽ\¿â…'€ã"À73	~.IÀ9ºrW5q@æ|®§GØ@[Yèÿˆ?üÂHÊt,ù¿âáê ó*/¿ã"±_ÞâÏ¿í@øM"Q¿åȀl¡êOTHERspp?y`Ð5ßf?'¾Á'^<'?ÖF
Y©D?Ñ®ij¶ù?äª7²Á27?Ñ݀¢P"?yB~Xý&
?•µ{¨?ØÓÆÒ4ì9?Ï!IŽ¼?ãc—š3—?ÏV{'ß.?­»û²æœ?žšßË©ž©?Ô\üÀ§X^?µˆ
ɓܑ?ãõÁï%g?¶NÆU܅ã?Šóš=ø¤ì?ŒêÑ}§ƒ?Òx ëÙ`?ÇT[;:?æ‹uF'0½?Ç]ï•Ï3FGL J1745.4-0754@2%ƒÀ€æ@%¦<OšÀ9ÿ}úâÀ;׎Ǯ€¿éòzv=Éå@õwæÁk?þ±Ø³iy¿é¢Å¿^ǃ¿Òïò¥¾.é¿×B5Ñëg¿át¨üì'ÓAGNbll?íÚ½¤ºV?Ǔû¡×6r?eyô•b¸?l¡ŠŽ6?¶uZn1'>?Ǎ¹Iæz?îO{Ü©œ?°"e"?xŸbË	?€±=?§ôb¸Ô6I?­Í—‹?ëÚN°¬?¨ó§9ƾ?Ÿ£G°e ?¹eqà&?¹Fs£Ù ?¤#l
i×?í3'õÐ?§Wµz?R*¬˜¤Ò?R
v1©?¶þÀÅîë?¦ü+ÚC33FGL J1745.5+1017@Alú€d>n@3BࡕçÀ9F–µ¹‹À;=4Ä,ë?øtþÂhDã@'žEzÞn?ý©ò!vr¿æњì¢L"¿×•&'¿âDîôàt¿î¶9ÀãWPSRPSR?Ÿ	Úf©D?œ‰ÆÓª?îK§Îù?¯*ºý¢G? JNu»Ë?©Azðå?¸N¸ oì?¼¬áQT(›?êƒ8†L}?Â!®3m	?³—Õ­,%?³Võä®°?Ä9"Ëؒê?®a¨ÖXyý?ç o~'ž?³ Ì$Ѐû?¾‰zx2Å??¥©ïµçƒr?Â\:1†??­*YPr™?æ™ðNm6?¹³½0&}Ð?ÌD"Äç?¯è hÜ÷3FGL J1745.6-2859c@vJ r~¿¤¾¿À`2À6	škP°òÀ8f€®I#?Ñ1뷕ûL@ä•Wëy`@'þ Œ=¿ç¥ìù'þu¿åõÁF†Í¿ß%áË·y¿åß äçuÅOTHERspp ?¢9z%N?­´b(­÷}?¶@…'äõ?ÁJ.Æt¹?ì
ê
?ÅL(ªOÄÙ?µ-ݝ{?¾à|Ä]oÌ?¥bù"œ?ª3­Ì±<?ì"ÜÌ,?ÁÍIŠ*ÊÖ?»o
J%?¨Ehû!a?½Ö¨~ø¨Ê?©´QçSs?èã½?¡¢?³`e59Ã?¡Í0:ã?±‹ÒÑý'?TP-jp1ˆ?\‹	fa§¿?îÙèg¸?±Ý›9Pž©3FGL J1745.7+3952@Pd™àvp@=	› æÀ:¨KAFò-À;Õ«ïÝs
?áû=ЕÉ@
= åRՐ?ú÷x_7H¿æ£…µOòJ¿ë‰IáZ¿Ú)ҝ'n?Պ`·áêQAGNbll?ïÚYéGBÿ?z¢,¯±®j?<g>œPäº?`¥SwG?q—r™qe?v0QüJ?ヲá!Þî?"'úHß?n-(èNx3?yCãÛ_áI?rúúéLò?v¦FÄot?ï	£à§Ù?‡äÐ|Tf?§ªlŒ8?v秈Ït?•øn´¾Ä?ƒ¦|«O8p?7C¿<?Š
qƒ¸Qo?D(8'ëî¬?aãµWú×?ŠM®¬'r?‰ÊŠŽâŽ3FGL J1746.3-2851c?à ÖdP¿ºh~À5 ÝÀ6‡7`ÆÀ8·*´ßp=@áhy@-5ŠÑTÇ?óËá'LË
?í}Â"¤Å¿Õ¿Ó?,» ¿äè‰÷e&Ë¿êO© ø³…OTHERpwn0?Cwq0z™Œ?EItÑ-?åtž zu?ÑÜ>ґX?Õ
rا?ÑÚ&"ò?`Œ¥Ö³ç?fT"
O?ÝT%Ô×Ö?˄¢^1K¥?áaIG>à.?˖`JF%?k$'	TH?ˆÍGié>¡?à–—§™i?¾*CŦê2?ÝÌg¬˜"?½yy×ê?dº"µ/Š?q+»È ôè?Å;ð]5"å?½Ek²dö?êœIT¢é˜?½Ù³e 3FGL J1746.8-3240@vO¿Î·‰ÀH?Z³ÖÀ7a<ðKWÀ:0ñ>œ@×Þ§À£Ê@ú§S@™Î@o$¥ü©¿ß}wŸžÁL¿âL2_Æ«¿è™»L
´S¿í<ôàg3kPSRPSR?$7õ"qÄ÷?"Ë*,µ?ïFYkî#ƒ?´¶Æ€%×?—b—¬*?¥Ð/Ò½3?*³x²3¬÷?D†€1'?ëÑí¦Ü¨±?¸'
iú––?À±œ†`ÐN?¸2§Ý¤?Ž R¨Ûu?…;J¢?éÜÜaO?´­Oò¶/Ÿ?Éևcìq?³ñ8ƒ_£?q8¢M5ö%?i5ˆ\™ûé?êei+Êr}?ª¨­~¹?Åà–>l†[?ª&÷Ë~‰(3FGL J1747.1+0139@:õ€`°@.FÓÀ9n‡Êd<ÀÀ;©¿Š¯¿àl
‰_©x@Ò[]@%ù?œx¿å]yfâüÔ¿çv4ËÊÕ¿èŠW+±¿ïþ÷'ò[RAGNbcu?éòààWFÖ?ľ2Ù»?§ÏCÏJg?¦Ba û?Â@«º/?ÃT}°
xû?ë륬Y÷?»uV5s?«/Ýì Å?ªš	?³SÜLÍ»?´ïI˜L2?èT#/?z?®{~ø9aV?¹z˜{? hÈ¡yg?Áòqbúô×?§RU<æßC?áßØØ"®Î?¿1g¶¡%ˆ?·è(jéÙã?²ãß6³?ÖFD5+í?¼æÛé—3FGL J1747.2-2958@vt´ ½¿ë@~ D¹À6rA&:ý,À9gåëoO@¾o›Cgß@bqŕ 
@yV-3??ÄéVäEíԿ丄&~Ÿ¿ç*‡ÿs,¿íœ‰8#PSRPSR?F»ùø²Ž?HlT2ƒ—??çøñQb¦?Ð[PÙÊ.Æ?Ñа a-Û?ÐVº†—æ"?+¥º¬Ï4?X(†ÑöÂ
?ç掙íõ¨?ÃS¯Ø¢?Ð/Wl¿?ÃSÑcŒ¬[?ˆ"â'ô|Ö?…(-àd5­?åCêy?¼Ú³%H?ÕÙÏj?¼ç4Áö™?`üÅiÍh%?ad³Èæn?áå00›OX?¾J\(‹Í?ܦõÆ?¾få$jöÉ3FGL J1747.6-4037@uâî_ú;›À˜Ü )€­À8Ü4mÅÖ9À;8>4îõ?ð{"§;™@¶ÇÖÃƔ@•¡ŸÍeN¿¨—ÌöúY¿äìȜÄû¿äâCåe¨"¿ì
tñÅÄPSRPSR?Áð/'œQZ?ºWnaøî•?ØÂasÒ×?Ì«!®t.Ê?ÞE†ÂîD|?Í( ×?À®…'–x?¼ï²ì–ô?ÖërB›š2?ÚäDSø?à^¥zqMH?ÆÛÐãw´?Ø,áè?µXQ"ºÝ?ÕZ'Ln©Ô?³dµ~š?Òxº q´D?²þôz§?ÍûîÜ#Ķ?£óèb}'"?Ö×h'g?¬œNÈ?Ú*ï)+Œ>?ª¿œkÇCÒ3FGL J1748.0-2447@¡v m³¸?û€à»AÀ7VãÉW,À:$GŠLá@ö‡`±ñ@JÁ"àL[?øQO¶ñï¿Í¤‰øóB¿ÞY bvÞ¿äðè géô¿í( 2:OTHERglc?…J£³œÀ?¤¿/Z
"?æ\¶ZÞO?ÍöëSÙÆY?ҝx†,¦|?Íع~ïv?‹j›€Ç¨í? Uñþê›+?åÙÀÐ?Çê¼ûº9Ñ?Óq*òYœ¤?ǜ^'…
å?£"|ûÏfN?˜‹txìýÔ?å£}ßK®ð?ºÓ~)jÞ?ÒF"¡îµU?¹¹ì_ñ´?•ý8#RWv?Š'0 7'?ãq
J_"v?¼«2}m"×?׾鳜?¼"AeÊ3FGL J1748.0+3405@M¬BŸ·ÀÌ@;.¦ÿ³©æÀ9œV÷]šÀ;É,¨Õv¿À(UR—Òo@†íð]÷@²ÍOÔ¿æ]ìÎ꽿ã—B•¿ç‡@fn'¿ÚI-è½æwAGNfsrq?ïî$ åÉ»?l˜DWj?S³ãGÙ¸7?Rþ@ÅÞ?PÚì'ÒN?jž&¿Ÿ?ïϵäºm"?'hzƖ¹?aŸŒ˜Ì?fbIòÂ?n«¸úQŸ?€'k`Žíþ?ï@È,z¢?†{î8Î?€õxwhÂ?t¨•söÌz?/ÿhà~?@íÍ:d(?ïèP;_°¬?jVéöÅþ>ìjZ£
f?KÆ'£œd?g"45ô°¬?j1õa}"Û3FGL J1748.6+7005@Y!ˆ M@>µ 6×-À7͙ȓ'(À;#Ö~ý6!¿²µ¹¶'à@õ΋"Çs@ƒäŸÒBØ¿àtæu¯¿á'À¦<¯¿àr|Ý~ÔO¿áªÀÐë‹AGNbll?ïþ.îEÖû?%C‰H—&?n²Ï{?Ѿ¤°?%5nî±fW?#³ó|K ¡?ïØC€Y¶­?v@¿ôj?^=<7?d9çT_ëÈ?h°áHOø?q]Z€½?ïRV
ž)c?ŒBº©f?sÔ‡ \?tÍwJ('Ý?ÍÉ,Xëz?‰"ÔaâNF?ïþ_@ýA?9¸®ãŠîn>"Ö.] >°¼órìf$?.O Øý[©?9·
U²¯Z3FGL J1748.9-2021@÷ŒÕ£5@TRRá#À7éèEÏÀ:"vOèu ?ß²žDÆzñ@‰Õ®óò@aŸØ"¿ãÊc0Q¤¿é~ùÞ1¤¿äy–ÄÓH¿îmÁBá&OTHERglc?Æq&
¡Î?¿Îù«ŒÍ4?ÍØ|½N^<?ÆB=ªŸÓ?âí—Mk?ý?Écë!6½ë?Æ%êIûèƒ?Ä»ùO¶Ø?ÖYԔǼ‰?ÈÙ
üôN?ޓ6F:O6?Ì%&G…,ó?ÑÊS¦D½?²doZÇ?ÐÊ<ÔHɏ?±øtT#BC?Þ0øØñ³?µß¿ÑÒ|&?ÁCüð—¼s?«pÿÚêÇ°?Ê@'\ejM?¹~'¥ŽÊG?åöìÀ¶P?½b…3FGL J1749.1+4322@Qi # –@=#ì_9K{À9
AðeXIÀ;¬ŽÁÏBÉ¿ùù"Œº8 @úVÆz@ù¬ƒ(¿â‡½m֔™¿åUifK
š¿Þ4
LùǛ¿è¨ú_­AGNbll?ïT¦)ó0??–´²OJ?p
 ä‹'?h¶F)1aö?'gùY`Õ<?" R«§bß? #K§?ŽW—Œ:Ep?u<Jl"?y=p¥Qª?žs£î
Ê?ˆ•ŸHR?í©$Ÿi4ì?¢ŽEõî?"Þ¶J·Ç?‰âŒõ"•?ªþZä$c?AۑF03?ïU1‹Ï´*?•Lå/¾Öd?DšW°òßÄ?ZwÞi²K?"´ûȁã©?"ú>ÒV³«3FGL J1750.2-3704@v^ FÇeÀ+_ª4œÀ8³¼Àæ½À:éÜF½S³?ï|@Lv@
hhîV	@³Öà¡ëοâÓíçпåjÑfe¿å¸ÜP'`¿ìˆ¡ú'+6OTHERglc?˜…\>Lz?•_2ƒQ?ÝC;H?ÌgmDšXn?àš7ši˜/?Ìb¾a	^ô?¡â³ÀTµŽ?¦"èúÌ?âRc´Ò¸v?ÂÜڈº|ð?ÙâOøc?Âô¤›ú—§?ÑôW ¾Ê?³-ža¹Z?Õ®oñéáÐ?´/Ñ\39S?Øћ¶u_f?¸7ã äŽ?ÁÐl@ŽJ<?£yaÈ]µ?ۛŽˆ ¶?±™y.ãî?Û|;WÒ,?±TÂðŽŠR3FGL J1751.5+0939@Avf H	"@1¦ý`OÀ7ù¢(´T0À;l5ç?úåÙ¡q@|Z
w¢@5÷Rñj¿Öp†Ҙ¿å=WÏ¿ã Áõ
¿èî>D´AGNbll?ïÛñÁ¥ ?xñIÜÜ£?U&°'YH?TEóð°ù?iŒ«ÀÍ?vüFùg¯y?ï³ËtIR®?ƒ²Q¬K-ä?kVTÂ?F?o'аðÄ?xozO‰h?~&Ù~æ7`?ë:ÙG4
Ï?ª¤×ÀšË??®095Ø?ž)€IU?·7QŽ"?¥F©Èç%Ô?îè@¾'³?MƒºhÜ?pt."?µ5?~²Ê-óÔ?žÚÜ¥/üO?›V{gó3FGL J1753.5-5010@udvâ—À'ù¶^À9Jûüe@ÌÀ;^&>?Ԁ‹"ò²S@9DM·ÃÑ@(Ððž¿ßk6cƒ ö¿ä뜋ýÈ¿éÊ°¤o¿ïÿÇo.¦AGNbcu?ïìD•²~_?dôq¦:G'?XÒ"¼Ú?`GÛX†ù"?MIœþ?RñàkD°?ï¹|PÌVú?ƒk–H{°?XL_$™Ê?aîä	hƒG?}.ÏÂ\?€£"IË ¥?íSqèõÝ?¡|T»DÙ?¬¡Ìì)ž?šÜ·˜Ô?¢˜ûõnx˜?#:ì6J¶?ï²ltм?Ð{ ÓòŸ?C¸(HÒ?N±óKû^º?'BÜÐGOp?~ ä8ð3FGL J1754.1+3212@LÞß¿î—ù@9j´M,ÙÀ7ôkõ oÀ:áNÊϝ?êÆ"Ì¿@Ú¾[?þl>ÙÚ¿Ýö?ý›÷˜¿Ü3
Ú¼¿ÚþE(‰Ñ¿Ýï¯f"AGNbll?ïûöX™÷?8…X&ÏÉ?6"ÍF" ?F%P—Qo?9?šޗŠ?5¦ UÉíü?ïÔýpÆ%?x‰x'Ú©?aÜËf}•±?gh,çi?j7(¼Ef?r¬Ëdÿ†?ïj…½'¹´?‡Ð8æ|?v΄M•?™?uaU²[J?‰÷Nx†óT?ƒ'ÏÝ\7?ïíÆÁ6ƒ6?e…ÏGõQ>éwün¢©;?ŠT=f¹?bÆÍ'î?en¶d˜Jº3FGL J1754.3-6424@t'ñ@ìFÀ2r?©c;À9Îw/†FÀ;­±¨"(?Óº0q.@[¹ïÐ\ú@«r`o¬`¿åø¬˜5&º¿äâƒ3ëXÿ蚓Ð4"ä¿á£¯ƒAGNbll?ﯤ'çuä?ƒz"`W?so褙?tÛÀfpÑ?u|# ñ¨?y¨®fßO…?ï>	ë?šÓ;ñ*á­?v4ÀɖÄ?f"!Žt?'¹Ò
Ð87?•³¿("܇?îÌOoË"é?Œ@š_Z?‰§Ýc&òä?x抇Ûå­?™¢#U)|?"Ø]ÁÒ$?îXï§è·Î?—qÒ,?{V+¦í?y@!ã?§C|;?–Ÿoà¬^Û3FGL J1756.3+5523@TßÞÛgš@=·™€o&)À:M‡rO©À;áËÜñ?Þ[ǤÍ\ó@o»îƒ*í?ÿ°ð`$ØÒ¿Ø/óÃ[´Ý¿ìn`mŠ?¢A>lTð{¿Ï÷Xš¼ýAGNbll?ïɹû¼~¨?~œd÷֎?Q0ñ¥‡­'?W{
Ü;?vÖŸ^ÀC?|¦G0Hf?ï}	ZIÍ¿?'QCÁ¬‰?€7=ô'?†afØ,Ь?€†©/˜?'¦5*IÄ?î¶$F8‡?Ž‰0¾NÝ?‹ôÀ²
f?ƒú¬_˜ç?›AiX–U?ˆAX'-?îÕGÉQ=?™€·7â?`¯Åt'k?zéx<ú?¡ ‡'#?˜?—õG3FGL J1756.9+7032@Y?'à°«@=ûßä׆À:Á#å¸VÀ;üˆµENJ¿äó|îí@§†³bîb?ûIÇÚñS¿í8~_\¿æ´
ýÁ§¿ÒÈ ukg¿É…\¾ÐhkAGNbll?ïùâà'ß?la»¢W4?3`R–?lòõñù?=â›w²ø?A'iæ-i?ïÆ~N?~÷ØzH?f¢°9Ð?k¬Ê">?qo² bÌg?wpt­?ïCeSuGè?ƒÿÆÚ³]?~>pÖ?vkÛ¤ó5»?¹ŒQM]?})-Õøø??ïˤ`›G??w¦/c¥ãS?
Òã1¤‰?iÍ(ˆ>?yø)ëú:ì?wž
ñj3FGL J1757.1+1533@D–uŸ¿Mˆ@2ߏ`Z³«À:-LBα©À;ŸÙ0ˆ^?ðY— ñ@q•înr@\"Dž?嘖Ät†¿Ø·§.¶){¿Þ™À&Ä¿ïÿÞ&çJ|AGNbcu?æ8 "eö?ÊfÖ·ÞR?Ñ×\X\#u?ɆšÕ7Ø?›v9DZ
?¢¢ÿ"\?ÔÇwK…¹?Ë6;?xÂ?â<ñG:Ì?ËmîãL»Š?ºþ$,˜½?¸¡ÂãÚ¢?àŽkfm?´Œ©"+q‰?Ö,t)ÂcH?´Ö'[òŠn?Ánýþáƒt?ªFÌ4¾}¯?Ù»'¸,‡¹?Àu¾;Àt¬?Ý¿:Ž?Ãô÷€®3?Á
Ôk¤{r?­œ|>[ïû3FGL J1757.4+6536@WÑÇ@0q¸@>?ÐàÀ: À
¡©À;þÀ°^×ý?Þ¦mV^u@¥'Ð&Ém@‰ãŸÍh¿é*š=¿ê[Ôþ…½«¿ëW°év?ãP0…•AGNbcu?ï‡Ֆ;?±KðXǃL?‡
E†¯Sü?±QçùIÕ^?l¿Ô¬t±?oÅ
"FÍ?ï»wÑG¾˜?Ql²ß?oWÉHûº?}ž ŠÊÜ?r˜2·£+o?"SÔ~\×Ë?îzm%ѓ³?•<	¸P?"G£8
d?Œä…e\¡?œj¸
¾-?‰çåËóߑ?ïÊHn¤ûÇ?ÑâMHf?@'ÑBȋs?XÍ÷¶$P?xÉn…)?‡œ?z|3FGL J1759.1-4822@u…|€"ÞÀ'ê"ßÎ1QÀ8þXÒ)- À;S&ìÓÓ?â×Hêæ¤u@×E¼wÀ@^%à9f(¿âö¬…ڿⶰdGŽp¿æ7ƞñƒw¿ærI@¾ÕAGNbcu?ïÖÐC筕?xœ©ƃ?V¾¡¤ôÛ?X7sí%3?mÐkFDq-?u6Ù -«R?ï·£
b4?'q|‰Sæm?VãV'?\Û€Í<?~ªsV$'\?€Æà'ÑUs?î–À´þ?'b[ºsF
?'I6ðk?…˜›KýÉ?šÞZIMn?…`'þÒ
œ?ïÁԟوk?y+u·.É)?-žu'¿?3u \_Y?~-"A°?xþðäœeS3FGL J1800.5+7827@['~¡Æ@=×ÿ/öhÀ7[M-°<À;>*ðn'…?"­B@EOÐwÒ@È@3KÝ¿ãnÒ]Qâ¿ã¡Â¨0¶+¿áÁ	¾«Ýû¿ä×¼Öú<AGNbll?ïùþ¾³?JEt ^¥?)0±të
(?+"X	;å©?A»"ªboý?G©Ó}ž?ïÓ¥2oö?yÉL˜%W?^ö'‹÷d?c'0'|?l߅r?t]¦°ó?îî(ë
þn?'¾ÒÛ¤ºÙ?|ïG†RÌ?})Îˁ•í?šÿ̾•?'/ݬrK?ïøs}©œâ?U»Ü0ìÙ">ÛNsˆ(sŽ>ïZJ·º80?Mûlr|$ì?Uµ@?·"C3FGL J1801.3-2326e@¬ÐDÑ¿ÐB OÅÀ5™þJZ"À9lžéd³@w¹ŸôR@mÁ̾Š?üßÎoU®¿ÑNŠ§ŽNã¿ãoNlt¿å;ÇÁË¿èÙRav½wOTHERSNR?§Ñ,(¿©Å?´G*´èw?¼V.ƒŠÒ?Äv׌éÆ?êø'm«$?Ç?9Bè?uÜæ'2ˆ?›œQ«£å(?âkÌS¦0 ?Ïp_ˆüÞ?ÚÔ7å–ö?ÏoœP¥g?³K™']Çî?§•÷÷2µ?Í݈±Ï?¶ÊàÄS?æPUk³ÚŽ?ºývŒM?{À/UJ?uè*û6¤?Ýáص.,¶?ÃÉû3ÖÕÂ?àÙ%
Èú?ì'mTŒ3FGL J1801.5+4403@Q»&ßÓ9Î@;þßnÀ9g½¨l›4À;ÍVØS錿ҐÑ4¡®w@¶6b½m@`M˜¿æ…$J?ÇÊ¿é¡[j'xœ¿ãéUͬW¿ïÿY,t°µAGNfsrq?ïü"×B¬ø?7ÁEwœ?âËq¬Â?•~p)hh?4×M7»ã5?5¨€¨ÊU?ïbÅ
ʟ?'êÞ}a?ƒÎÈö¦1.?~œ¤9Æfo?ƒô'ç&ñ?…ÿÅ@.f?ï_.'"<?€åÀR"ˆ?ƒ.Úix?tê6'Ñ'?"³G@²¸í?tgyÿšI?îî÷1$[?˜õ?˜w?}‰oA?ƒu\ÛêH?š¹º÷ÿ¯>?"¡e½ú»3FGL J1802.6-3940@v`—ÌÀ ٍ0À7?ep!À:žT~ÝU±?ýaÛQÊÍï@ç%=§*@ñVe'V¿ß·w=ׯ‡¿ån~P›"¿äEdNM¿è ÑxFýYAGNfsrq?ï?áLµ¡é?˜tDé?[Pz­.
È?bOáËSÖ2?–NξxâH?˜#h(¨C?ïu0»?¦cnF.ÚI?m}1'¹c?†Q©÷hÐÓ?™!·‡°‡0?£æQÊþcÂ?ëŽ}N¾Ák?©Ïqâ´I?¤rÀ÷þ´?–&[þ1u?¹Rµ
òI?¤þf¢Ô?ïß .$6í?w½ƒÙËè?¤¸—÷,þ?Kj=›tZ?o¢¬	Z½?wOü…§ô3FGL J1803.1-2147@ U,î‡Þ?ÊÔ)`T18À7!DҗçéÀ9º[‡SZ@ªu
Iè@¥öy|Ä?ùÍBM­\ð?ïýǯ½®ˆ¿à*Cùb¿àÀfÂ#Gû¿ì¯–kÅSPSRPSR?\{=ÏñúØ?nrƒ'¦3X?ÕûÀnÍcÖ?Ðx¡ˆ»H?äóâ)±U?Ð|é"ü
?I
ôEsÈ?m·Ê±,ü?ÛZƒ#­:Ä?ΐ\Ùö?âL{±%QA?ΙΊš7á?‰#ê'8k#?…Ÿ…¨‰¡?áû¾H^wG?ÀË،4®?Û?d±N?¿|$ðš‰?isđß?yßKÝMV?×ÿÉ\ªÃi?Á[­r5ç´?ãºu'˜VÐ?Áƒ2ÁQ3FGL J1804.1+0341@>Ô}`}ï@(h³Þ¿=˜À9í´ùqp†À;^èÅP׉¿Ô¹öP©»¦@Ò´WàçŒ@xÀ†‡¿ã' »Ä3C¿å¶ŠE"²û¿ß¿
º9¿æ›kFÜ«AGNfsrq?ï²Ý"ïV?†yóæ¯í?;r_S_?:ë­<—M~?'m‰@O™?†2Fø9R?îö²g±þ?§­¶2°g3?n?é§+–Ü?vmXÓÆ)0?aÁþ$MT?¥é›h¦£?îÄJ‡QÏK?–éÀõ)?'µêJßÒ?yâ›×?Ÿ¾?žoT  ¦®?'—lL_Ê©?ï;tì?Šæä*Õ+%??¿­"??mûƒï¥{?›¸Ó4'Õ?Š"x@'l3FGL J1805.6-2136e@!5\ ¿Êû@?W¦'À6O«ºbgÀ9yºZÚA*?ü>ÐJZÂ@ì}'%VÒ?ü³~'W0¿Ò"ŸÅÒ=¿áñëjFÆ¿âõѨԠ¿äóEšOTHERSNR?‹O ù¨C?×År½òÖ?gMÌô'u-?x"O_‰?ï{s¯$Í~?'â>'êð?ŽIõ\±@è? ]:Ó½Â?´}J?Hì?³*_Yt£?ì÷.â¬1à?¶
Ž4Žds?¸ñ¢Ö´Ë?¨K_îŒ??±ënûú¡?ž;˜Ýt‰í?ê¤]Ū$(?­°ÔTiøp?£– Ø	"(?Ÿ(‡ñçþ÷?±Ääì˜h?§M©ñj?ìùrAÓ¯?®s§)û«3FGL J1805.9+0614@@­çÖyõ@)矾vÉÀ9ìŽÐè»@À;£ŸM7Á7?÷x&º©ß@
'ë¡?Ë¥Öé±4?Û¨¢þiŸM¿ÈÁV8¾.ò¿à«ñ«uÜ¿í-b
çPSRpsr?¤č•?´Ì.Æ
q7?æ©Ä~òTÑ?ÑÜ_;d]p?Ð*^phµ®?ÐÅK¨žIÉ?´Þqj[?¾"³l ª³?çCMS>S¸?ËtS¦J?ȃ¿*Íûð?ȘÕÝJ6Á?ÀޟQDþ?¬3E9¢¨©?çkDõð%æ?¶¢^cþ?Â5
ˆî#n?°úE©A4Ù?ÐÆ3è`ð?ÃyBÝüå?ፈ;'ƒ?ÈS_š?È=xð* ?ÂèÖb11Ç3FGL J1806.7+6949@Yñà'Œ7@=-SaÅÀ7÷Þ¡
§#À;Zë´ï`v?ð-3¢Câ-@^!p¾0@ßGŸ¦Îá¿Ý‰V)q,W¿äp¡1'GÝ¿ãOK Î}b¿äë]ö͞¦AGNbll?ï÷z¤ê_?G¦±ÝD:Ì?<ysR—¼?7K">.?CÚ×Ã8×?Aªº–›¼?ï»Lä¬6O?€}ÔG…??np=+ªí?o†;-¯?sXU‹Oµ?xidžÁ†Î?ï%¶;Iex?'ö$Ò$?ƒÕ»¥n?|·YÍðô?'^[
š?†®«Ønƒ?ï7i4Ý,N?˜©x
Ý«ö?i¶"`n?jë³z[?•ò5ˆ
2?˜)¼ˆ}õ3FGL J1807.5-4343@uÓÞ²gÇÀ&9@LzÀ9è6°–5aÀ;xcNƒñ'?ñ&>Þb ‡@î)#øÁ@ö<À$È·?Ñ$Š#¿ÔBÖÿ«œQ¿á~?kOÚ3¿ïÿÞý¦ßROTHERglc?ÁX§‰‰¥Ç?ÀüŽ9.¦+?諜=n?Ãàš±>:¤?·ñÏ|ñ?¸–«G%KS?·òÑV©Ù?¿lÉcw?ç¨Óð{cî?Å?ÒSt?ÅÏ6Õg\?ÀÛŸ¤?ØZBßÈíÈ?¶qØÇxéS?ޞ"–â7Í?·Ek%ãÄ?ÂS©´Õ?©eIµ¥8?Æàè~5?³Xb†mcž?å–-§?¿þsF\ÿª?ÂÇI¸»0?±Šò9‡É3FGL J1807.8+6427@W†À
¡©@<ó?ÀàÀ:žQ>ÌÄÀ<èÙrÍ}¿õ"§èö@Dt¤@½_€C1X¿É¯…°꪿à*:ø4Á¿â0@ÔÓÎÁ¿Ø#hÖ¿PAGNbcu?ïñžy¿J¿?‡Ùx€œ­\?ZuA4üß?‡Ö*˵ø ?"nZcs¨?!Á߱đ?ïÐ[d¼¢ˆ?y õÁŒÙò?b2Jã'P?gùuú³€?mrP_Û^¦?rx«ð.èã?ï'"WkÊ?'…«ñz?'€Ôú* ?;	O»Î¬?ƒ5Ѧ0¹S?uq®¢íö?ïòmj¯=©?[àÕf?æ>ðÖŸ®ÍX>÷dó(sfï?ZáÒ[ón?[½¢ð'R®3FGL J1807.8-5011@uuIàâiÀ,?{@À:¦Ë±DÀ;xût€¿ìäkWšy@înKbª@X+Àx*´¿â%Ÿ¿èðj¿D,¿è ·§exï¿Ë†)žÎ¦…AGNfsrq?ïåÚ§'z?fK"d‡ß?Kø0ý㒟?Q9æÉKš?c'L/þ|?aS•^T§Z?ïÆ@Ö~n¬?{‹Š•MM]?Rôäôrxl?XàE²ò¿I?x"[ƒ¬s?x)k§Õ‹?ï" öŠ­ß?ƒP\ð@^?€Õª®ï:?r­¡Zb?"Q×2»•?}ä¸Ï6êb?ïªÆžHk?zö+ÚÛ?e]ï	³û?oô½Òå?…7ó['?zñòR¬Ù3FGL J1808.0+4652@R'³`<Î@:'
4fÀ:ÄIqcÀ;ððÄXŠ¿¶C²"b¼Ÿ@¸Šh#Tï?û¤h_dêe¿ïyATõP?ïi†âðµ¿Û+ý¥Ãڜ¿Ó'ë=Œc·AGNbll?ïù'?þ?Q𹏝=?<
²w¶æ?<XŸã¹—?;!y%ð?K-‡Ê>Y?ï¨
×áW%?"ˆjҞÿ?u^YÖ~©f?}-Yn!œ?vœ:8ÕÄ?x֖µÞ8?ïNâØQQ?€$'ú5?'sq6rô*?v…Üb@qŸ?‰Ô
x·Q?rÓ¥¹wå1?ï",+TbÉ?†I•ŸKÎ?{–‰øê
Q?zwˆÓõ?zS`\ä'(?€¿¾«Ó3FGL J1808.5-1952@$ê;¡–¾?£z"`h®<À7֓vié©À9´rcÊ«?ù¥)Gwý@¶ktBG"?ým¤ˆµñ"¿ä»?܎â¿Õܾ²Wց¿çíß¡»§¿é!& þ'ÃOTHERglc?UAt+=ù?P›Nµ×{?Øz%!9Å?Ðg[C'o?ã¸X3YĎ?ÐjQ4n÷?üQÎ
¢á?ŒNBc7¸{?Ð7SgH²I?ß$j"õí?çœe#pP?Ãþ_÷tüÐ?¤$?'T—ø?"Â
åïE¡?×MÞ–‰˜?»ˆ*À~pK?ãô?qµ?»9"ÿÏWh?¤ôc¾Êµn?¥=='ª"=?Ìúáòªš?»Ù¨\)ƒ?çrGh®$?À¹ËÊf3FGL J1809.4+2040@G¬Ì W"ý@2:X@2õ÷À:2@ºˆ'À;¥:Ùâ)?ÜR!ñþpÅ@
·‰Ð£Æï?þ)¡-¿ä¨©¶—¿íõfß捜?ݜ—¡ƒ;¿ÆìàϟKFAGNbll?ï½å‰"°;?Š)ÍxÅç½?3QËS?8€(¬>?Ø)™oíÓ?‰ùGIÂ?ï¸Ý Ð8?"OòñC?eSÆ휇?kqªøÌe?y-¸ÉßÆ?€uÈ,¬ñŒ?îË6îñ?Ž"IéF6?-@ùyl?ræ|¯(?žv˜¥e?Œ$h'"ùÕ?ï 4"³JŽ?š¯‰­§3.?("ÇæÃß?Eçd71Ê?›ÈGÙÉ&¯?š©š0ďE3FGL J1809.7+2909@Kás 
Ìã@5F(ÿӊVÀ9
3èdØÈÀ;Lü~¹D?剞C™Õ @×Ú Ÿó?þ}a?5¿Ûéß¿Ø
‡ñ"޿ۊIþYj]¿ÜÜÇÊ7$AGNbll?ïõî½lÞ*?W?ŽF®¯??ÑvK¸M?9€ã5y°?H\Oá~¿?TÜ^±\?ï¡»³{Ò?‰S6ÎzTJ?rU~›?oú¤ns?|̨2ùìž?…¶@áÄž?ïJdWÁ…?…l:ٞó?ƒ/á4*ÜÁ?~Ï«þ™ãu?ŠNµäÂ,?{?Ö:E×V?î4Ô5Œ?™_—lÞ¨9?y³Ó鯢p?wR½Í"Í@?«Æ;¥†²ú?˜N"óLz3FGL J1809.8-2332@^_±ÁYÀ˜Ÿô|"À5†·¯.VUÀ9Ñ쌅´à@E»ÕX·|@MØÈÙx,@®'oXÓV¿Õ.™1%"5¿à¤Øðz/¿å6KÕQ¼Ç¿ìÆ'ŽmÊPSRPSR?AaD;?%0Ñ8©?ïœ&0kC?ž1*‡'?ˆáW2ƒëM?žÛ›†¯?Š#€u×È?@áVÈцY?í։ÓbÀ?º¶¿Y(ވ?±H #\ÛE?º·åº‰=2?j¢µÞßU?h´ÚÃ÷x?ìá´¥Š´?§! >€Y?¸aý$³^?¦Â'‹yn÷>êDG™¡' >ù†Ö§"¡?ï•ä1ÓÎû?ˆO¦H?Š€by%Ù?ˆH&ÙFÌ{3FGL J1810.1-1910@&">'âÆ?§Q*?ô«œÀ8w~@w¿TÀ9ÄõǗ٦¿ý~™Îr¿:@œˆjÈê@ÅT`)‹j?ïKæ'øm¿êý
!P² ¿à9õÅšç¿äˆc`øh\OTHERspp?p^á×+¼Œ?s›Èú?]3?E­Uaêdà?RÆs~—ä‡?ïÙÖæù-í?u©¶±."?Çøð£Tº?γظ w?'
)¬ÄŽ?˜Ö‡H£DL?éuC…ÝkU?θiÛ©)‡?ÁO[Õo_?ª0…Ƀ–?«æn·ä?—±×Ÿù?éáE=˜Ó?®yo_ß2?Ú\?ìL?ÐObÀ\‰?'ÈÖ[•?&ÅHËÔÅH?âÑ¡ÃDÈ?ÐOñž"63FGL J1810.5+1743@FNÌ W"ý@0Îs`Iì³À8…Í!†b…À;Q€J=:ô?ýû%Þ
¥@––'7þ@ÅN¢zhÒ¿à–X¿äjlÊ9¿æÒS¬âˆ¿îùU=8ŸPSRPSR?¡ÇáÌý?¡ø˾£2h?îA"¢æß?²ZóÊ}?šèӗ?«f({§?˜"•h#vV?¥] ™`ÍU?í^OòçK?·cµ*G?­Ñ6~2?²‰¹)é`?ǔÞM?±ü×]è?çDᩐ™v?´Ò²Ä™R-?¶¯6uo/»?žmÔ¯µ?¡UZ´è?'¬Z€2?í%Mù‰?¦6"vÆãù?­HT^²—?¡ÂæÎO3FGL J1810.8+1609@E"©Ÿ¡—@0$™ù;À9Xˊ­mŒÀ;Zˆú%7?ãp+¶s@#»DLÊ@ۇß\òI?ëLøWÙÊ{¿æ/™"9ƒ.¿Ü–æ°N¿æi$nÔ AGNbll?ï=Õf®?¥û­Ïæ‹?o–ÕüÃ?O?pŽ¢HÚ?"R…<zÂ=?¥Dó…""?í¬7
·–"?¹{^YTë?'}»µ84?–Þúä×¼%?«ý±Jú¤?·1
ꯩ?îEåzûÉ?šK'N¬
?ódŸ?¿2ƒ¦G'?£R®ÇA=;?–¤´ÉJå?éœjÔ³"?³rÜH"Vê?žª0QÊú?'æó¢±]?Ź¢ú?²½Ù\LhH3FGL J1811.2+0340@?¢æ_E	õ@%8žç·4À9Hê7.jÀ;"nÞ,µ?òî«¢°š@b}¤ñfŠ?û\zßð&?ïâ]¨QÃA?ÃT…µ®oŒ¿Ð}‡0Fªð¿àå…é—†AGNbll?í®âF'œŽ?¬ûœ,!BD?¢l3(_Ђ?ž÷ôu¸x?¢¥¨ovf"?¤ó·¤^×?êš]ú2I?ÆZ û¢ç?²YŽ"‰	»?¹4ÿ>0•?½!ží¥cý?Á!ÅÐY<?èA€tאx?²h³g£å?¼KA;=ä?¤Þ
Ó8?Àë،,?­hUǘ?æBì]{ù?½IØ0ž??¿Ôìî¹?´Þ$Ñ?Ç
FV³—?¸YNsŸ3FGL J1811.3-1927c@&Cù¡A-È¿Ôñ·€
IÀ8iǾp¸À9¼ÑÇÞPƒ?ìÓNà҂@לã{@áŠÿ¢âî¿çOhË?ç~œóÁ-\¿áú©êIµV¿èpË¡ÖªOTHERspp ?ƒôòZ͜?‡¶LËÀ|¾?Ä:$£qš(?ÇT>ŸŸ©?ê¡£
¸c?ÇòN†ñ_?ÍwŠ«sdT?ÒwΗ&ÊA?ØâûŽ"!Ì?ÒJKFÛÜ1?Øa?Â,
?ÔiÙñqÔ?–\߬De?©}'\a¹í?Æ·L´˜‡?®UÝP*ìx?åÔºôçÈÅ?³DÆQV~£?ÄBLéÅ^/?Áy‹v'f?Öä•Èù^í?ÉÓ<饹?ÞúCÂ#ñù?Єi{`Ë53FGL J1813.4-1246@1>`ºTû@ˆ•_ùõÀ6¹"ñkéÀ9àЉð@±CÄÐÔï@ÜúE€èž@68õ¿à*¿Þû‡Ë:ü¿å"P3Áoï¿è @*8n¿îE;­nýSPSRPSR?X!%þ?f½Åa6§U?ì­ÓXVv?Ä îú¤ü¯?º1§S?ÄðA"úÅ?%­Ñ¯8ãÉ?BHÉ=dtŠ?îeܞ#qç?©°9µ_Å¢?©ŒˆL¨·?©¯/í	#Æ?›l@A
<F?'ö''¶?ä¥J?K?»ýóÿ
ª?Ôþ§}º–?»|¦Wµð?ª_Ñ?Àd·.?ïݺ›?–ZôóÅMu?vX³µeQ?–P¨…9‹3FGL J1813.6+0614@A»®²@&x¾áQ¿À9JEµì¶wÀ;:,XN?í¡Ô¬rÂÉ@st¤íŠ²?þW@-†?ï©
o6¿ÃWû'e¦V¿ÜPMR÷§J¿áî2|÷CæAGNbll?ï¿?o˜ú'ÜX?I؇V?Oèsܑ6û?U؀>.ã?lþ²*sÂì?îT:ÍòRä?°Xe•?Š3;£Í	n?›Wê©c?¤/"7珌?«2uÂ^Ü?í҇xhÃ?œ³´±­ò?›¬®/Ùúr?Ž'º¶Ë?¥1a†Ñ¥?•óæRw܃?ìöÎND?¯ãð¥?œ{¼%'?•mÛÞñKn?¸Á" YD'?­¦?8®Y3FGL J1813.6+3143@MU§€)Ú@5Y‰?¯BxÀ95†S€À;…¿üñý?õÐq‡¿@ð`±¿Ÿ?ú­ròe㊿ÕWøÿi¿ß¯ˆ:Ãí¢¿ç(´Ù¿àÇæ|²iZAGNbll?íŽn6ïç-?°¹÷cKÁu?¦U$W]ò–?¥^ñBƒøù? Ãø9£š ?¥Z>äa!§?î+yÿô¸Ø?¯ÿ›wàƒ,? öR–ýx?§a5—¼è?˜¤ÓmôÇ? JB'Íu?éÛga©â?°ï¦ÎËÃ?ÁŸ »5îù?©gÛtU?´*ãN†Ó?¢»ã#ÁÓ?é3g
"R?´ç ¨»º¢?»ï|¶[A?²C6ÑÒ?»QJÝ3?¯÷µoÕã3FGL J1816.5+4512@R6¢Àh¡@8Àæ_E	õÀ9"¤úö«ÃÀ;µ(Ùº?úDن@p…qœ@äe½Ÿ¿×-ó´±è¿à0Pÿ³0¿ãꯋ?Ü¿ìÊ9­~[ƒPSRPSR?s•ÇÄ%Ã?uØu··W?ïno&>{Ø?•òc{Ýs?Š™Rîþ÷?'Qûùþß?™ÕÜ·
/×?¡7èÑ €û?î¾úŒ$?¯¨Ëñ6DÄ?¢Ù!û¸¦™?¨ˆp®‰?·C
'¡ö±?£¾ò³ÐTð?ê‹ÆSþ;?¨Gx\?´^ÂS¾n?™@äT欗?²fFwIæj?¡Ö,ê®"?ì1VtIÍ2?ª	x€–›|?¨ÌÏ`?žÓG3FGL J1816.9-4944@u† fèÀ.X­~«À9ülhÞæ«À;Ë?'‡]?ö
´ynÖÍ@·Ýª»ú?í{xg«ñò?ïGãmðjÙ¿Û0!œõ¿ååÏA"•–¿ïþ'B)'˜AGNbcu?är›{Ùé?ÎøB{Û?ÈåoìÃ`?ÈStŒ±f´?ÅP#•M"ø?ȔÎýU‹?äåewÎø?Ñû@¾<¬9?ÍiƒbLÁ°?Ì	¬ûhÿ[?'çÔq?À¥J¯?]'?ØU—ÈZqn?µ]f.Ä¹?Ùî:Æå¶B?µó§.>ÄL?ËxZá°¢?³¹Td8b?æ7&@º·E?Â¥Ù·j1¶?ÈdêÄþ"v?¿ùZkJ*?½|øp.î?¸610ŸÊ3FGL J1817.2-1739@*Ç$ß³Y^¿æ-£€Š#À8@5¾þ­ðÀ9î'Iü?óEêmFª^@ŸŸšm@+/ŸÕÈÊ?å´õ«gâ¿æ˜"üS£¿á8½`É¿èš´¡²ÂµOTHERspp?¢`DÏW´y?¦VšTÍÓØ?À†¥;fé°?ÂF³·
"#?ê¸Rd0ÊK?Ä[QMÓ%?±ñ³2?¾ аíÜ?¸ÜŠ&	òO?¹8NLxU?ê¦Mר[t?Äs—/´¯;?¹ò=ö»ß?¦½•hÐî?ÄÀï¼ÍŽš?±ôI	'¢?ç'|Qõ8½?´ƒ¡§›Ÿ­?ÁmÒ±2Ÿ?¸oDiw÷?£±©rVf'?™òõƤÎ?êi´.Lö?º¤ÂóÃ×3FGL J1818.6+0903@B¯¸Ÿï0@&¿ãAƒXÀ8¾Š¯ñʳÀ;0žHUh¿íû¨V@wEöÚ<w@ð6îÍ©¿ã69Àk¡¿ãÆX¶È¿ç.«'5>s¿ã+h¸óswAGNfsrq?ïÏòÛÄȕ?vÆéÓo6–?Z'{ÄôÑÄ?Yœ²az?qb3,^€Þ?sF	™þæ?î×!Q£ü?¤úÅÆ+Ê?nèƶñd?r'%í(-Ó? Ÿ^ƒ–¯ç?¤ŽZ
D3?î£Aë.?™éü ,Íø?"2.iÃT?ˆ~
Á;à?¤¥.–ÿ¢þ?"ˆ>tݛk?îèÂB?"ýþ²Ûa?G"È­¸{I?SM—úÉÙ?¡!0¹'m?"Ú`º€^‰3FGL J1818.7-1528@.ù"!bPW?ƒþèÀ(½¤À7söLø×À9 Š(Ž"@þê<F'@Ipû@?ýr9΂Úe¿ÃQ²º§Ü(¿æ>ÕÈôÐø¿è¼*2	h¿êÖ#ú±OTHERspp@?¦dW'ìï?²Þ¬ýR¶?™×ˆa›Ý?­xЅbb?íÊþG613?»RÂOú,â?¶¶ÃhfÉ?ż£™?»r«û?¹$îíÇw?éÈùOøá'?ÈD·Nr·	?À²¯`u+?¬ZMÚ©$Ä?ÊäYül?±­Øû×M?å{Qc›?¶¾ù`@?­S+³å?©Wþ?Áp"֕©?¸íkéŽG?éËZ—ŸW?¼ƒ)½¹ð)3FGL J1819.1+2134@H'ŸÀ$GÞ@0}>ö?À9å(¡ù¤À;Š¦8
‡¿¼KŠÔ&¿@'ÈVñSj@¨_Û÷¿á֟ÞÏ{¿ãè½YDóX¿äv'6+"µ¿²^B¸XÃÞAGNbcu?îSõ-&?°kÙ݅D?'=Q$¶øó?¦ñÈ
YD?¦?Üe¿om?¨Äñûk~?ïÄ3`Ð?"^é<ï?gpV"iÊ?mñ1Ýæy?'ݹkÂñy?'XÇOìX?îBCö-L?™€¯Ê`?•7™/£Ä?…¢Í3¯$?¥`(ÖYU?'ȇ	}ƒ?ïF©ÃŸŠ?ŠzVi?Gí°ÆÅ
;?Qo*áÍh?–kZ•æc?‰¬2â‰!3FGL J1819.1+4259@Q©'ŸÐ€@7¸ß_vˆÀ:<³Þ¿=˜À;ΌQ²z;¿Öô&žáhK@¥²YY·@߃]ÿålòÊÀᐿî'ÜDÓ³`?ÚuYÂØÆð¿éü½ðˆ`.AGNbcu?ïÌE(;ï ?Î\¾Ï?C.¶P»C6?P4f*h«?ww•ðÇ7?~TTÞÍ?ï—N\¢5p?•ôàá?toœ‹äz?{˜Bv¡Ú?é5#Î[?ÏӕÍF?îQ5¹ê
?–HÏrïÎ(?T‰?'¿oÄK?£&N˜¿6þ?'b«Ã¡±g?ïJïÝgLÜ?˜
j¼?4Í&ŽIjK?RÜ+rÛ?–NϸÝ>Ú?˜Kƒr°ò3FGL J1820.3+3625@Oõð ¬ @5'â_ܪÀ:m&!Ò¸ŸÀ;ÓùrGE¿ã>ªCF7@x¹ÖÐܧ?ümá?¥¿æcÝ	ñ_¿æ¶[[	f¿Ö'÷6‹_ù?¾d´AˆAGNbcu?ï÷ù‡+
x?MÄáðâ?›@îÓ?×á:m¦?LƁðâÞ?L¾[*??ï»GÕ³PÇ?'"ÊÚižv?eAW§&?qОÒ§?w»†ú"‹?ŽHë¢Z{?ïIf4Å>?€|—{²/0?z•BO×Ö?n£ÒÔ±Ç^?"","b\?{k{`ã?ïÂ&îLÞ?|xºVÊþ~?"Àvl"? ÆÕcu7?~³aul¸?|mµ÷H3FGL J1822.1-7051@t:gÿyÈÀ7.L`*ãÀ9õågÎEÀ;«¸ÕŸf?ÆG^™‹@EôZƒG@Ÿ¦ e¦"¿çµ¾t´ È¿éJÐeUË¿æ	c3´–¿ïÿƒ£žÃAGNbcu?ïhVO=¿î?–ÛCËðÁ"?qåÒ&Ûsü?|TMVzâ>?Œ÷ƒ"J"?"Ö"8
¬Z?Úús#	?Ëë_•µÖ?׌éӉÈ?Èeu†ƒd`?Êò)r¦¤]?¿r»³_»?ë}"0BŅ?¦ýRŒ$Áˆ?­7ïSܞ?–´zY™Hì?µwâ†?å…?¢1a&‡ÿ?Ý)'1øÎ?½y¡^=X?Ñð9%A?¾ßë‰=J?ÑÊøè"áò?º§¾G+¶3FGL J1823.4+6857@XÌm_êKc@;­5@S­&À9`žc,öÀ;Æ\>'ãÀ^ÙH0Em@¬àÑ;œc@DI€§…@¿ä™Wž'>ñ¿åFfËÞ\º¿ÞZ'qf¨3¿ë!Hï ùAGNbll?ë8Ɂ·Æ?»Áµ9=iœ?¢¡G.
ƺ?SE	ûÜi?¼é[:ë®?¹ÍUž?ï™2ˆ…®›?"$'1^¦?r·ªþ껏?{ñ"'.öÑ?€Wˆ_û]?'8NæfÒ÷?ëy­¢ËÿÞ?«²h!gÓ?±PIà1ÀÏ? Éïݽƒ?²âI	n@=?Ÿ÷ÈU0ô=?ïœm0]:?ŒîtŽoe?-ÈSçbi&?NߐË*®?ˆ'CdK( ?ŒÎ}òÒQŒ3FGL J1823.6-3453@vjá€M˜9À#Þ\ÀjTÀ8ƒè!¼é*À:ۚânõ?ì÷lN˜ûu@àóÇ™?ûùI þ?•jy³íz¿Óoò:îé¿Ó¾Òƒp'¿Ý«xÊþ&ÈAGNbcu?ìsÊzj?µ=šÉ'pœ?"G.ðü?…æaX3W ?¹Øɶf
,?´Pl˜;p'?êV³æ'ïö?Ä6‰ÝHn¨?ž°.ΐ?¡ýaým¼K?Âäº_õæT?Ár¥¡"ì?é{î`ٖÙ?°.FH1»?§\-"Œm?'ÐäK*Ä?Ä9;;¸?­ç^l?åEÅ»`^?³(a)ºu?—臹 b?•yXÖºŸ?Óõídï=?²ÙÞ$œ§3FGL J1823.7-3019@'œÿT´bÀŸ!€nÅÀ8ÜMÂ*²[À;&œKû?ì)¯‹žY@
þ{uí@yoÿl\J¿Ò>ÕÁp«Â¿áôôç0¿ä8úC8Ë	¿ê'ÖwŠ?PSRPSR?ÐØ"Ï©Jè?µœ"îœï?ÌÑõñèç}?Ã7"Gìí?à_q± ­?È%9ô­{k?Ó&péCôm?˟3SÍ'½?ÓóÖ¥á±k?ŲþÙN?Øå¸pÚZ'?ÈP^ԁ?âÜnUíþ?µFFe<Åp?ÉAùDÜãd?¬™O5{"q?ËLMck"%?­0Ø)^Åï?Ðíx¡ÖQ?®h¯£EêQ?ÓÞ@åC?³ðÈ	Î?Û4FÀD,#?´.	$¿†3FGL J1824.0+1017@CŒß€-·É@%g‹_D36À9®TDZ±À;a~B%>~?óîÔâø@²¦Ú?ÿ×>€C\K¿·O£°•Ä¿Û»vžAôí¿×agnN<N¿îQo3òÿDPSRpsr?»—ó­<o?· É@NýZ?êg{?½,xrúåq?±+zƒj'?°ú[=t?ÙáÔ·Ú>.?̂ؤƒÿÚ?ÖÇӕy?Æú¿ÀFü°?ή&€¤X®?Ť›$	›?͐²Wä{Á?²—§X T?äv¯ÕçY?µÿ[‡´Ç?À"ŽP~í?©'˜5·}?à™wœQG?»¬4ØnjT?ѶŽ·i?¿VˆRüP.?ˌDæqL?±C†ånuè3FGL J1824.2+5649@UnGßþù@:ÀÁ%ÐÀ8Iò×sÀ;‰ùÖñý?趃Q¹±@%͙ü@@®?Æ ¿ääÛ3a=¿åŸÿ«±¿çQIß/¶¿é‡pu«ÒAGNbll?ïï'5 ?iSt9ŽÏ‰?U›õs•A??_·…ߌ?H,Daõ?UYHŒö؝?ïÉq
»¡Ã?|ü{ƃãm?ek¢­.<é?iÇR"™ûŠ?p'§Ë˜L?u:ï"N=í?ïN³7ü
Ý?…hÎÄiò¹?€Aƒ½ÿÎT?v´¶þȜ?Œ®BüºŽ?4«Èê®?ﺹ¬ƒ¯Ã?"2˜™
NG?QDšé‰Ó?TªGÓ³{&?~R=m»?ƒÊïï³­D3FGL J1824.4+4310@QÇß 'á@6ÙÙb¶®À:Íú8?ânÀ;øIlÊ.?ӕˆª€i@
"mã]\ý?û˜ÔÀ6;{¿ïÐwwclj?ïëé‹Û|#¿Ü P¤Õ"N¿×Œ0Nk6ÊAGNbcu?ïðÐkíB?X­¨S™F?PãςJ^a?U&"FÈä?Jö±G.9«?ĚN9?îyCm8E±?¬wB‡vM?Ÿ¦ÀºÄм?¦(D¸ã°y?'0ў2y?—Ý¢C{y?ï/¬œ‰³F?ƒü#G扶?…ïÁ®£(m?}p…#Y¢%?Ž%.ðP?w5½¯"ÿ?ì®>0æ¾?°ü¸¼µ-#?µùUxàE#?°ÅÕ®ßE!?'Rãÿ§'"?­Ý4}Iñ3FGL J1824.5-1351e@1'A@<02¿Ý`às%oÀ6Œn~bÜnÀ9*Š§ŽNã?öWvšÙ@'
äµvÅ?ËÝJ9pJQ¿ØèPKqîZ?é«\ÚÌiÐ?à(‰¡~ëC¿Â²_8IÈOTHERPWN?ŸçÑ&æì?²i?÷YQl?Í3k ú"?Ð9·»´Û?ç³æŽŠBð?НÜ<	¤?Å2t#	ð+?Ò:¦˜Óyw?²Û(âŸóP?¼•DðkJ?èWýÚ酋?Òï˜05Å?Å&J¼U?°^æXBZF?Á_ّkbô?¦æl¹Ä?æc	ø.?³%ÝÃëZ?ÀÏ5ê?Ç2?^"^R?çþÞ?´ÇÅp¢ž?êìŒDÃÊ-?Ëgš=îŽÐ3FGL J1824.6-2451@DHÿÎ+òÀa'ßÂó°À8E3å	ÚtÀ:Û5ƒo‹©?ü×È j® @ ½Ã@@"4"¿Ù­`Ç|<"¿ãs§ªyª¿åýÎl+™®¿îb!%û£`PSRPSR?_ÜäsSŸu?bidzRÂ?éÕåÿ'h?ÄYÙýùJÙ?Èh¯(?ÄEY¥Ãþ'?Q¬[qýoÝ?f£üÅX?ê è]ï@½?ºúz',?ÅYÑ_,?ºö~*¸Ÿ?¯FmØÛ<M?¡«ñè?çMú"<	g?³Mî×xPE?Êöz<ÙR?±§õU<×J?'¾ÛYd	X?'zF=wº?êökmî¢?¨4ÍÍd;é?ÁîxÄP?¥•:š í¤3FGL J1825.2-5230@udS_ôöÀ1w?› 'À8Óû|ÀÙÀ;Z*¤ï82?õŸ©X~qJ@óE$Í>ã?þTK'ôà¿Ñô]%†2›¿ä]rÍä
<¿æ˜ëK#¿ä±Çã%AGNbcu?ïçàl¡ç\?fQØ4 ;?NûnJao?VAÍz»0¸?``·Ë'‹N?^>Ž,Lö¶?ï¼^pbN¨?'ýœ¢Øzv?W6Ž{Z{™?^JSû˜!?|$0
•?€ˆX	j8?ì§ì4|vÕ?£%Ñwcu?¨¦Ó[]?™Ù;?¬Úi\Ûs±?›u?ï¢öCe;X?"¾pfÍ?C2aÿ5?KÈ}Xõ?†I½Ðû?ƒÅõSšÃ3FGL J1826.1-1256@2Žwß4®]¿ØJä@m»À5š'3K†çÀ9y[ñ˜^@	o_F6›@™åX3ô@ÃTUýŽ¿ÕmW=mc¿âš !¯¨¿æ嵕3êy¿îj+.¤O¢PSRPSR?
h°\\Ù?Ö×ioCË?ï/œ¿°ˆ?¨'M#í;?™ýÉ/ÛäÙ?¨µv¾F?"àØυQ?IOxWÝË¿?îG"ÚG¦æ?ªZH¥£vÑ?«sÒI¬Â?ª`¦ËSÎ?nQ†s?n‡kjóˆ«?ë=.$œ?±e¬iï›?"Iß[?°û3rðýþ?®mp+\? lçêœ?íÕô¤G?
?¦l‹­]¡?±IïBiüò?¦hÙ!©"Ò3FGL J1826.2-1450@0â³ÀŒLª¿ô³b ‰!ýÀ5þl3/uÀ9ÂQvYS?úȉ+bYf@º¯¾Ê@å¿ÉY$ß¿ãº/§î¿æâƒb ‰"¿éÑQa£Ê¿éh'žùTëOTHERHMB?‰2½:ƒ?‰{>ß"œ?ÙÜo¦¤?ѐMb«|?ã…%SB§?ѐ/»×y?^;ˆYIû?z>Ê3S®?åüÕ¼¸?Ê`K±pK?Ô¿Ëwû=?Êäýªþ?ÀWÄ­'€?¨÷¡µÃ?Õ¦BÚleÇ?·5)L'_?áažl|?¸[ê­Ï"?‡á	Ú­¢?†α6Ž/?Ü	"‹ÜÙ?ÄØl+C)?á›ê•ºÜ?Ä»cßCŤ3FGL J1828.4-1121@47	 :2+¿ÁËTŸþÀ7×ñ
õ´À9×!éBN?ö*mþ¶)@P
º?<@kÛ±í¿Ç´5§+Óm¿çN'D~ˆ¿ì½­?h˛¿ïÿkOÚ2çOTHERspp
?ÂQŠ¾4'?Ä­úuQz?±Qç†Ö[?¸É5Bà?éA`Žu¯°?Êñi灦>?'!Qãí"?œ(r›÷ð?µi/xè"?²Gïr˜CÞ?ìÉόø†?´ri¨Ó??ÆB÷ϸ?°d7¤ëâñ?ÈqÕ9њ?®A²|£ú˜?ä\çÌë׬?µtž¦Ã{(?º§¯šr">?³¿~½Ñx˜?À®ÝI@lS?¸ì×ÓXÀ8?èRºa £?À±í'•V¤3FGL J1828.9-2417@!Ž¡à×ÀÚ{þÀ92t]ŸîGÀ;r«G¿ñàÝ"Zrè@U<Kv?ÿÃÁá6fD¿ë9Ó>'5¿ÑÆ3îˆÎ¿áŸ‰¤X
¿Ø{Úp=CœAGNbcu?íŠc#^?´'n¼Æš?v‹åT?'2óm?²FH¯¦‹>?³ïÃ~ò<?î£_jÕ?«I¿…ïŸ?qWÎoM¨?{'Z%GžŠ?£Ÿ.õ«hó?¨ò‹@R©?ëPÿüò­?©>eFß2?¦$A"Õü?"èAZ¾º‰?ºeßNԂ?¤$äüB>?힤~ä9?¥Z©ÌP§?@å6\'0?GG¾Œtš"?²éœ'§þ?¥V>ÛmQ3FGL J1829.4+5402@T·W?íUÙ@8Ê	?Câ®À9§0IAÀ;¶½ã$þ¿ÚFØRM;@´
Öó—<?þè`·Ð¼¿àjï7/í¿à—j,Õ²¿àº-°3ÜH¿ÍÁ:Áa›AGNbll?ïÜâJª®ù?p¡žLišw?QQ
4g(Ò?T$œ"Ù?ju.»r{?l«¹Œ¦Ô?ï¿\dž}‰?Ëº,@4?e'pÑ>î?jÁ°Žå°>?u•a؜Æ?{xìÊ([q?ïíÖQOõ?ˆCµb?…çh5"Ê?yz"† ?'.'öÏ?€^MCHþ?ï'êò:Qt?™sÕÈ.Ÿ?5ª‡EóE¨?<AV"Öë?Š×ï7<	!?}gBæ«O3FGL J1829.6+4844@SNü_Ìï1@7|5_]]©À8®¥|%ëLÀ;™—û3èe?æH¢R(@eàÚv@뮟e5¿ãoÉ´i~Ÿ¿årcÎö6—¿æ 4=tU¿é¨e¾´AGNssrq?ïâá]~ËÄ?f‹:=µ %?_WɈôr?X÷Ö|Wzn?Zå{ytg¡?]~²Õ²kK?ïR{¯?À?Óš»kg‹?†b["Þùí?'jØN/ê1?…ÅQï?‡l}›êD?ïFê+½×Ž?"u'!Û4d?€¤"êO(>?tù¸(/–€? ð&:óØ?~¢þgÎcx?î8ç¸i?¡^[K®r\?'c²¾]¯ù?‡3)¬bȊ?£NÒU¡^?ŸÉF›°b¨3FGL J1829.7-1304@2ÚB×P´¿ó|ÔÂ^À8d"_õIÀ:&²ò0?óYœƒÙ¾Î@̼¥BÉ@öc«Kž¿ÓR|¤–LÞ¿Ù¤Ò}ö¿çw,ò§Qé¿æ‹(³OTHERspp?zC{vи2?u—DÖ©m?׎EŸí—?Ñbµ3<Jª?äV9žÄ?ÑdwßøºJ?³à})T?½³²my­R?ÑÖ=õêvi?΋›"hЏ?ä˜Ñ_à3?ÐCâF¡I?ºoýË\?¢Ë">*05?е٩2µ
?±òØ5íð
?äW‰í9ù?³Sѽ@zÆ?¿*Eß18?´\ÜaëG?Χÿ2Y$?´Fj=oã?ç7wƒ?¾•ÞS«3FGL J1829.8+1328@EQÅÑqw@%ŸàAׁÀ9øŽ½À;e×F£R€¿Ë×¹"Sš@
]|DÊ	y?ýîÞÀX¿è|ãN¦?Å"›-¿äž,÷b€0¿Ü£³Úž­¼AGNbll?í½€	ø?¶;AÓ~D?€RF†ª?Ó¦3(‰ø?°Û.â?µŽW´¥ó?îOSü«ÛG?°»"²ô]?'^pÀ|8h?'3#›ì'?¦s$#=i?­É­|ß'?íѦ,y?  xQƒX?"NóšMA'?"§'C0x{?¨¾#kGÍû?šöø¼ùT»?î5!ô!‹'?šøх¥Ü–?ƒo.±º]Z?œIö}Ÿ?§Òx°•?š1pð(33FGL J1830.0-4439@uâ!€M˜9À.Oó v,­À8ÌÌ#Y¡\À;q¦½n‹?öê—é@Jô@c‰ô5–@&þûɧ¿áun°Ñˆ¿æN­q+«¿êT@([‹8¿ïÿ˜ßé#AGNbcu?ï×GÙ=Yl?rŒÃÃ#€?jCÆFmV?lñi'86?\èÀù"M¬?^Ã+å-?ïoÎçÓe—?"v€Ü`Ý?oƙÎù ?vÉÑK"B5?ŒŸ—£[Ð?Ž³¹:¾=?í?¡^r?¡Ý´þôâ4?«tìœS¾?™ê¼Ï)YZ? y‰MÅ5?'må4mAó?îÓQ¾©*?›)ö¸E+?…ºÇëm?ˆRî®Û7?š¸d}Þå?—3å;qàü3FGL J1830.1+0617@B"}@XGßèˆjÀ8³È
Jk^À;	óžÈ®?ë‡	t¦x®@Éý &¼@â.Ÿ¥¢;¿Ü's'Xi¿Ý·íø@˜÷¿áÁ¼öƒ"¿æ¨GúÀ{AGNfsrq?ﮘ;'D_?†¤ÿA
Þ?L[ÊÜ;?Ká$jÐ`?'"4y''«?…Ûƒˆ3œ4?ïÙݝ¼
?¡ó/†±ðÕ?h~Œsq"?l"ÕJÑ0?œ¤tzº£?¡9‡N4ûn?í©Aõ³®? µ'²¹«€?• Öä%+Œ?Šâò{´í×?ª›u4â/Z?šû-à<ƒv?ï|¹557™?ˆ9ÚýÁþ?BtÌ@Ž?G>Ì8áès?°keîr?‡¼n˜ÞÒ3FGL J1831.0-2714@]ä ()ÀÑkÕÎ(À9§™¼ÕÀ;1«.íSU¿ØäƒÒï@IA;3²µ@°ãŸø†¿é"çN5ö¿àÔs·þ¿ä¹¸w͎`¿á'.ohAGNbcu?íËVø`ó?±A7ÿÛ<{?‹ÎÏQ%S?áõ÷§,?¬VÜ¥µK?°t™ñ0«?ê­d†Kê?ĺSüš÷k?˜ü¥Oó4?¥'ÙÖø?Â*Ú÷èiÔ?ÁvŠß`¿?ëËñnP	¿?§þ¡ES3?¤dY?'šB´«v?·ne	Ó#û?£AØ,œ{/?êyuKª]y?±Å앲Ï?x1ñ÷;H?v㻯_ê?ÅX¢9ÆÐA?±ªÿÅ®ª)3FGL J1833.5-1033@5'° F\¿ìU'?Æ$ÎÀ7Bo§WÈ>À9öáP?óæ¢̙¡@B¤ë1g@#ßâSG¿æɸµ™¿ã"ݧ)hô¿ç>EžMf¿è–¥ôEãPSRPSR?~Z0©j¬>?zï¡0wÄo?ÜÒéîplö?О¬Ü»G?áYÖ§tô,?Р8çkÞ7?'`/ç¼ ?›C·eil®?Ò¶ Lz|»?ʹý‰¯õ?æZªY"°?Ëh°<¶jÚ?­Þ¿w;ûY?™Ç•ï21?ѯ˅@ñy?¶ùU•?åJ.Eëǎ?¸CR8¥?ªî<\ꇃ?¢ÇDžéçh?Å×) ïS¸?±žž =¨]?èÛQÑõ'š?¶a7¡«Úð3FGL J1833.6-2103@(UΞ^$yÀÒBß·7À5ü#ü^ŠÐÀ:bÁ'ïV?ÿ,ý|BØ@ ø1T‹È@†Ó8¡²¿ãæ‡Ä–µ¿çWȋA«¿çÍ~d´à¿éZïŠfö¯AGNfsrq?îÆ$ÏÁ? ‹?r–
Ç?…ã¿"]Ø&?ŠTtìÿÝz?œK;œXâ'?AÐêà	"?î8­_š4?¼9©*Ð?gr{k£ï?©®Ý&?¨MgÖ\?¸¼›è"}*?çï:WPé?°×Æ	¯vJ?¹½5—(e‰?¦LFÏØ+?Ãd{×+µ–?ªãôw3?ïÜz0 È?'wT±yä?/G(wâ?E›Ú½ì?qj*'½ú|?'ls°3FGL J1833.9-0711@8‰¡_`¸§?âðÐ $ž×À7øUŽU™À9¦''ØÛ?ÍÂkä™@¡eç»eœ@ÙþÀ9ì`¿ÐÁaߙ¿äŽ8ýÍu¿¿æ†BCÇU¿ÚõâûbatOTHERspp?˜Ê4Uá֞? :Qoì?r9w_—¨•?Ìqè'T?ï;n'Áû?¢'šË''m?¶·"ÈB!?ÁoÁ<"z??'ýÇô¦Ýû?—WÞFÈ¿z?ì™'R"ì?ÁÀ9[¥Ì%?Á¸ÅD,%£?¬2¼é+?¸Ò"šŽý?£È1¦¼?èw|;±"·?±}uäË
?ÛúGWt ¯?Ë4TMÕz?T²Ö"ݐ?ZPš½ÑæZ?áø'é7e:?Ë.R>y3FGL J1834.5-0841@7HT`ªdÿÌïû_ :ÍÀ7]öÌz—vÀ9ئ²†Ði¿Û'ÝèÍx@-Ì^'Ýh@]é jƒ¬¿ÐP´ƒ)댿á¶`]Õ¿à'¿zÔ²t¿æOó]ZNOTHERsnr?Ž|0È$dž?Dwêô¸?"=~ÏÎ?¡p¥ÈY§?îì&Øî–d?¥¸y¢ÿÏn?¤±ÜWÉl?±.Àj›Ö? 0ªJ­=?¢ÛÁ
¡?í±×›/¯?¶W…ðÔ?²àyëŽÄ?¡,aîH?¬†@Š{¬"?–em"Ãt´?ëåßèÓ^?¥ùÄZwñ?Ï©BVŒ®Ì?ÄÐÉt4-­?u­ýý«+‰?|¸k@cy®?çêSna}ö?Ń;Ʀ53FGL J1834.6-0659@8ÍtŸå
5?àºÇà˜ÿÀ7Ã6ù'PöÀ9ˆ2芘u?"2ÛçYz@IŸæ姺@cߣê¿ë.°:Ê?ÓN˜~çf¬¿ÝV¦?oV¥¿à­èÛ÷OTHERspp?ÉnLE(?Å( :?¹ÓÒ{^?»<í»³¤?æ"2tf'»?ËêmŽ´ƒö?ÕVø?՝Lû¨]?ªÝrÊün?¶ü¸m^=?ãÍýЖà½?Õ~ز.Ÿ•?ÄÏÓ+ƒ_}?®'«¿ãS?Äß8ú!³?±m1­H¬?å"<ö_³?µ¦8ÎÉÿ?Ó"¿ƒõŸ?Í.Ñ0¬^!?Š‹Žvá?Ž{uª·:?æ‡fe½?Í×ñ2=•3FGL J1835.4+1349@EÇç@™Å@#}1(ùÀ9ÍMüUyÀ;@'¿aª?¿Çâþx§—Å@Ä¿6@¯r_Ãßé?Õ	j¤Zp¿ë'_º6'¿à { ŠN£¿í¨Î¥êà´AGNbcu?æcÏõwú?Ê¡—"'«]?§*LJýé?¤å
Ò\(Ï?ÐçîÖµnp?ÊrƒV¹¯?ë3¼_«ª'?¯,·Ð?™Nì¹i?¢uÖÛNU ?À0þz3k?Àô;p‡ÜÓ?çŠòKƒÂ?²e¶†F7y?½5†¥…öH?¢­/®§X?Ã9r°õØ?­£Š–Ú'?è.SpTò1?´°.1DÛ9?'†07gnç?Š{J!Fˆœ?Íì7¿I]?´–Ún‡®¸3FGL J1835.7-3258?øß}ž¼C=À&¾S‹'À9áB'[sÀ;¨±gìxd?øN{ÞÓ@ñæ"©r?ð2^צÅ|¿Ñ×Öì
¶¿Ý•»~ã¿éœolŸe‹¿ïÿ\×qk}OTHERglc?†"È^YÊ?&/zU®?êlÁP(&?É,"Ô)Ë7?ÄêÎ9½ÂÇ?ÈÆcg"?|°ÕNۇ?˜ÛïIÎ0Ö?ë6;gh>?¿\–)ÕÉD?ÁOGU
Ô?½cÅã¦Áñ?¼Zy¿Pàa?§´âƒ6Á?éNCȒ%Ÿ?±´}à¶ÿ?¹3güòŸ?£@jAD?y?µTŽßdâ?«‹ë-m;:?꘲-ˆš ?·äÅ£;!Ñ?µæcÛÊ$?°¨«Êpm
3FGL J1836.2+5925@V8tÿñ½G@8ÿ'¿°"˜À5<³»ƒÏ-À:YÌÅ@'@ oa6Ò@Րà?õ:€nû5k¿¿NšlÓ=¿Ûʬ"y
¿æ*Ü#,¿î¨Hî}ÃóPSRPSR?0´[ô$ë?0ƒHu,ëÒ?ïÓþî?¬­ºiߥÉ?œ°ͽÛ?¬¨x4Iã?RÎ,ìõ(?s¢ÇF®?ï—gçÖ? EzÛ®ð?‡øŒw(kñ?P¨??¡cb²qE·?šÌ¤˜š.¬?ìwOÕ»éš?¥Z¶áâÙ?³"ÏøèQ? ·],Ƕ>½M¼yÈm>Ï^C`ó?ïùea?RT	ú+§+?KçݨÑk?RK[¿qJú3FGL J1836.3+3137@N/sßË­@0É'àÙìÀ9_Ñöy}À;t.QZ¿³ˆœ•N;@Upõ¶@ÅxÀ01K¿è"¼R"®ù¿á†¢®7­¹¿æοë+¿äÅ4
^ôAGNbll?ïé<&|pß?kì¼åˆH?ShA2üµ?R>4M?ZlJÅëDO?h&Ò	\"?ï°¤zo$‰?"-ÃÝéþ?hzÖ5m[Î?k,®Ë*?{pW­·K?€å˾ÃÍ_?ï §Õ£1?‹]߯ÜC?…u^՟Øò?~ÑaªFr?'0UàÉñÙ?'Øh±Ïš.?ïL)ðƌM?†ÿÀœ]ž?V,k/§¶?S&²2Ql?•û4>+ß?†Bösÿ<ž3FGL J1836.5-0655e@9áj("?Ád]?Ô´ÖÀ6ñÖ³Ö\À9K~Íey¿õ«µPy@l«…Th7?ÿv
`:Ó;?ïŸíp±C¿ã2dkºc>¿ä5»wà¿ÐÞC\vyOTHERPWN?¬
vÚÁ?`?³Y8@DÀ?œ½Œ¼52˜?´6Cue†?íY<,rBu?¿E,ä[Æ?À³FÍÕË?Ê&$YÍ!÷?'l‡tÒ¥ï?›§9½ö&?ëGÊä$?ÊZùäa´?·$7 F¨?¥Kæ`u5S?´ðÁš»m?¢4¥Kl?ê}WõŸ½?«Í"±|?ÓÁ6"Ðå[?Ì~(''‹?2ŒwsÒ´ƒ?Iÿ¶	SIp?æ&©ü?̀¶ûî@ï3FGL J1837.9-0607@9ò€Æ^?ÈÎ_âáÀ7à~SÂõ³À9‡¨ÖM?óêy¶O\ß@ô.·x|¾@"BÀCý[¿ìNùõœF¿×Tj*Kâ¿çfjÆÙ~ó¿çYG·y©dPSRPSR?{ðsA;É?·g|‡€Ï?Í%‰™óÁ6?˵Tt@?è8œ;?ËÞBQ›X?¨G©—Å{3?¸4t`î'?¿œ³rAª?¿-'î6ï?ê‡îø;s
?Ä=®QE"?°¶ž3IÆ?_CEnö›?ÌÙý‹¡:?µ^¹$£sm?æ²®©R.y?¶´§Yÿ;œ?®ýÌúÕ¥?²!œˆ˜.?³[PˌM?¬@
Õ0`?뤹ì˜ö?»}îHv3FGL J1838.5-6006@tõýç!À5½v Í|À:$Âî&¹¨À;¨¶urrä?íuúÅn@2E³"k?ý´Ü€žöÑ¿â6wM‹Æ¿Ô€[j3ûZ¿Ø3Tq­}¿â€åC!ÆAGNbcu?îöc#«?¤8{Šn"N?qT£NŠ?u§s¾žP?œî†ž#w
?£¢¥?îKÝd
Ñ^?¨iÌÜ]A;?'+îhC‰Æ?˜?‰µM?¢,2‹1%&?¡{Î'£t?ìÒ6«?¨`¸\ó38?¢¨Óý)?"øÓD\? ?°@epž?¡¬s"?ìÉ
BKE?¦"X"jâÈ?œ˜‡ó•e?˜›§?·ã³ðÀ‡?¡dÓ~ÞÛA3FGL J1838.8+4802@S<b?û˜'@5ÔC@ÇplÀ8öïÕ'À;BL¨O??ԟ|EºŽ@¤%D24?üåâDhæ¿ãEÑøGq¿ØýÁ†óyµ¿×bÝÈë0¿ÖŽ¥nRÝ·AGNbll?ï÷I"?I!à{Fˆq?1­×h>O?*¿²—ä†?JÄ9Á""?F?ۂJ>ö?︊£ÀÏ«?~8Qëô.j?m²{"rï?l#ê¹j?tápUðl?wÐÇÔÛXm?ï\×}êß
?'´21ëg?sއþ&?z'0TºB?‰1AI*O?y<ºae"º?î…÷³ge?'…7E$¡!?^¹~…ÖÕ ?`%Ùq¾Â?¦¸TšÓ?',X+ƒ&x3FGL J1838.9-0537@:€o_3l>?Êxßl>À6ŽãðÕÀ'À9>áÃÔև@¦`Ž@
Ì]ÓG?ÿ}³Áä¿Ò˜b0Œ¿åÈmÈì~ª¿ã…j²SŽ¿ìІ^1PSRPSR?G	Jœ±ïè?N'Ž—è€?ʅµX[š?Í¿ñ㐷ß?éXÐWAìü?ÍÇ¥Rª0¤?òRHûÙ? )R¶¸n?럆•Wùm?¼)
Ê·v?Á€v…5Ã?¼˜åºT?–Ø\Ò
°?àzF]?Ýjuɘ·?¹€+n°®Y?à"4æÊþ?¹{î~µM?<¿‰‰?AÑJÞ¿¤N?à›1û'&?ÈEÈ>±x?ÞÂmÿǛP?ÈLSD>)L3FGL J1840.1-0412@;å`Ÿ}i?â£t?ܨ§À7«À_AÀ9Íúꉯ?õ{*ˆ"¹‹@?­le@Sõ?ݐ"¿âgrÕàqÅ¿èƒÝRu¿æß0$˜;¿ë"Ï"gˆûOTHERspp?X™+'ÍWë?Z#Pڒw/?á8A.qxË?ґ‡ü5u?ÝväwŠA?ҐÐYú¡É?yvíõë›?¤ìa˜Ö ý?âj(65z?Íéª^®±?ÚÅÓÛ¾:š?Í_¢ûÔ?°mý':ø¼?š›Ú}Ñ´<?Ø¥.̵þ?´ºŒzëG:?៶6REé?¶G:Vs=?~T?äƀ?~ÙxU,?ÔÖ=ˆ¡j¿?ÄrD|""?åX8»å½ ?Ä؁•¸ý3FGL J1840.9-0532e@:ËÂ@ÐO¿Ékd'õµÀ6¦rKPÀ9FS£C^?†è×sñ@ÙÀ»¡V?ü㪟PgÌ?ÖzwéDR¿½EÁ\\¿ÜàÝÓNq¿ßϓ¼
êOTHERPWN?£`Uá`™?§©»|ÖJ?j¿´n??w6¥>µ\º?î¯ãâ;}‰?¨ÏB!¾Í$?ÄÞèÎBZã?ÌáÀÆ9²•?"š"[Ïæ?š?IüéU¬?ê#t¹–êÈ?Í#-ˆù0?ÅЖØ8(?±Ÿ¬¸æ#? 
?Om-?qýƒ¶U"?é‹$%S%?²D^i™ù?ÌË䗉¡?ÆB‹ñxj¥?hÛuæâé?nˆEöóŠ?èæñó:®?Æ_Š¾Öª3FGL J1841.2+2910@M8"€,á
@-É0ŸÚü:À9ØÏL
ÑÀ;`,ÖøŸ¹¿íό‰Š@
Ž¨'ƒ?ùóÀ+©§¿ê2þÄZ|<¿áÖ©Ôò'‹¿ãijù—03?×ûîwUnAGNbcu?ìí¿‹Ÿ¾æ?À™Ïê"(?`wØI[?_l ®R+?¸
ä?À?ÀŽŽÈØô?ï€&Pj¶"?š"É´Â?eiÖΧßå?q/skcѱ?Š›ö1¨cY?—þk²`Æ?íë˜!ç€?›Á¼äÍþ?"1Gù7ù?…'"²Eu¢?§-ó½'<?–»[ öL@?ï‹n«v¢?	ÇÇÛ>þÔâaù?áGѽ¤?cñ§?åhJ<3FGL J1841.7+3218@N¾'?ßéà@/úÖ 2¥oÀ9J±ÓLBÏÀ;i»Þh¿ðôFn#t#@¿nëE3@v>ËLo?ÑÑ£=S¿è¿èiÜ̳¿Ý9"ûƒƒ¿ÈYÀÛÒÏAGNbll?ïOih¼g×?§¨eïÈä?R¿ Ÿf{¸?QŠ~¾?"æàÞ|"?¦ôHWO
?ïnüàØ)?ŸÅÎTR?b†­]'a?h+~Ë=»J?ºgò•Y?žîDõQÚ¼?îiûÓ<!j?˜Zú¦Iå?‰à㖙?·?¶A"ð?¢è	旙u?•xlå"[?ï^À–`†Ö?ˆ—è#HÙ?£ŽµHßã?z:Ÿ_¾?"I¥9Üo?ˆöî.ß3FGL J1842.3-5841@u?«ºÀ5Ë{_ò®ßÀ9È*"yÀ;~¾|§ñ?ÒCP@y¿@
»?ÏM?û ÷ÿ«q]?îÓ
;°bç¿ãÔÃRis%¿Æ[h…`¿Ý
7+÷eäAGNbcu?ïåå}¢?j!Oj017?4ˆàL•Â?7!*lôè‹?g‰ØxÛo?iûw'?ï£öþy´½?†Iz9/?`ã·ƒIÕ?cò"÷H
Æ?'Ézó±þ?ƒ'ßý†?ï§$©Å?†jô£!÷Î?"¬|-î?vx:R;b?•4àsÔ;.?€Òþ- þ?íµ*ÂÓ)#?¤—lj˜1?UP²a'u?_á$"‹¥?²iâ0à?¤g3ˈ@â3FGL J1842.8+6810@X£Óßæ…@9ÕiÀú)À:-¼±Ì–FÀ;¬à‹Ær@¿ðiö¾¸¸@wd/¥µ@jrà_Ý¿ãgŒ"S¿é´µÜ<ε¿ãNtžîî¿âì?œ€²KAGNfsrq?ïûÁ¾®+í?=1ajîf>ÿÉgžáêE>ü*µ§ž½??õt²'C?<t+'Æ?ïÐ
‰/QÊ?xÉûÜoÚË?aŽ§7éÍ?e:/Eÿ?nfϘÅW?s•JKˆ¥ú?ï…—#*Ä?zÙTŽÈÏÍ?lÏA/É$ü?[]'¦BÛ?‡ˆIëC?xS‡¯™?ïÓ7ߙ"ë?k3þa_d?	n–'êC>?
mqh¬£?v13¶?k`3ÖS‡3FGL J1843.6-1114@6
€_5ð}À,ß?ëþ@À8¥
¿cíÀ:š`' ×?ò— rç(C@DO‰€ï@ϔÀkëa¿áyÁùCñ¿êi¢'¿ìþ]YÙe¿ïÿzö…ÍPSRPSR?Âi+QÈA¿?Áõš]¹?½׿×$?ÀÀ];ÖF?çš3"ì?Ë
ÞA‡>˜?jYS?–ñ1)ú)z?æw1q'*f?ÆÏ{/^ñò?ғó¸ÍAè?Æ(Æc̛%?Å/sšù?©È•0µ?Ѷäèú¡>?°ðZˆËŽî?áÝÁ®œ*c?³Îm­ª-¢?"€ãî'ÚÅ?ŒöÐ"Îe?äI°{aF?òùQìÄ?Ö$ÊZö?Ã^ŒDr3FGL J1844.1+5709@U­aÿÏX˜@7z—¿¤ÆÀ9»J>³‡À;ÃhEc·_?Â%¿Í_ïª@Ó¤'UÛ@\ 'F¿¿áê£Åê0¿ã3xV¿ãµÝúòz¿ïýÎ xµ7AGNbll?î1=û("?¥ÁHü¨"?¢'O«å²? ³¯Ÿ›|{?•ŠNaC0f?""ÜX±z?í-Jw?®Î^Œ¿?®!CJ¢Ò^?¦1ß$‡.Ù?ž9h'n?žšE¥"?í_'·?¢&ÒG†?¬øwŸBD?œ†:×ÛÁi?¡ÖrnBJ?Tha¬l?ëóàgh»4?¬K«ç"E«?°ŽiI®£ñ?¥uŸK9?¯¥&öæ? b—æHe3FGL J1844.3+1547@G&	_ûZ@!RaՈ]À8ºë"ùÀ;µ}û®b?èqP¾ù@'L(!²,@9v7]d¿Ùnÿmš‰¿×¦on*ˆ¿â›®rÕÆ­¿â W·³\AGNbcu?îH–j)i?§b§·ëŒƒ?Œ<¿Á2GÕ?‰t<[é[?¤gim!÷"?¤v'ð?éÈ
†()?ÃâW"8?«œè½Ál?ª¸'7?Áø¶J/?¿È{µÁ¦?ë¹{PR²Ó?¨Ç×ó¿Î:?¨Ã‡,?–½å¥RÖ?µÒ¤ö&ãT?¢¹utˆW½?ä[ÚÜÕÛ?­Ö"º&¢?·®'<_F?¦þìÜ4?Ñ\¥·ü<x?ªˆu²¼ÚÖ3FGL J1846.3+0919@DX[_¢'@j!€-aãÀ8l|ÚF2À;$î?
\@üɦ&Ž@Mn=p3?îe@×\?¡þöÉ(0(¿³',²Ä¢¿á±Sißl¸¿ì…0-Å5)PSRPSR?u¹Ó¿­q±?{"É¿¡Ðº?ïK©s <?¡Ûô‰	?'\¬0œ ? Òê'ü2?'̃,Oç"?µóÊy©x?ê¨ÍfQ?Ä[þ€·øØ?Ã&TfdiÇ?Â?¸tþ¯¤? FtúQZ£?•!>2÷ï?ëS¯ts#?¨T¨é°‡?½?Iß>9Î?¥e‹FôØ?–ÑÜ&X¦Ù? Q*¿°^?íOAË]?©('8ï"?¯¢õ7{F?¥Æ5›ÿ9³3FGL J1848.1-4230@vó¾ýÀ1cŸVqýÀ:)+rt'À;ŠS².»Õ?àAšƒhC¥@
n¦9R?ÿ8ÿ€SLƒ?ï2_zÜ6š¿ã¡[Dý¾¿Ùd¦ÙÚ8¿åb©a§~£AGNbcu?îœYçÞî?«i½ÈQv?izunY1?u=óºd;y?¤¨™è›+{?©¹í€ú7?îhçOêÁ¨?ªåÓ¦D?:¶Ö‡²"?'õ&?¡T/–1?¤5ÿü%[?î/g)qÕ?—VçˆÛC?"Ғ…L<?…ú2›2?£}$¬Ì|?6Ï'y(?蹢ߺØJ?²O½Êw3?®)ý¤6©?•ç†~oU?Éc¯A`?±M©¹NDö3FGL J1848.4+3216@Oˆ M@-[ç^jÀ8&	Ñ:×À:_ÙuQ»´À
˜wDŽ¥@p'º}ý@JÇ?Åí¿éªî
¾à¿Ü&âå4o¿æ´Ô¹]⽿äVžÙZµêAGNFSRQ?¤Ú¢?"t…iZ½ß?edž	hÀ?nyjÿ?‡guFó Î?'´Ob!
?ï"ËÄß=?ž´L³(0v?\/Ð,ø?fÉ|]¤?‹GD	)0©?ž˽£.?és8ԍðÅ?°#nod"?±5ŽnÛÌ?¡ÑD—?Á˜UvZV°?«OîÝ@Ú×?ïòi™¶¸7?gWÝ ¨	>–*€÷þD>"#;¶¥'?[+iêŽAú?gWÕÚ쳘3FGL J1848.9+4247@RÁð`P@2{_L–²À:i»dgÀ;¹ZúøYC?èéQ×|î@ G"g{d?úV¾|'¿îÃò¯Ø¿ÇJÀ©º	b¿éµ¶¯]Ò?åwÈ/üiAGNbll?ï¾kº"Z?'ŸOé®A?{yâZã—?xÎ{ QÃ?UAŽËR?]•SZ#?ï›2ëwÆ?šÕ9–î ê?sÆö_R?‡ÈÊù	Š?~Ÿ"Wåí?'æÞó?îÛò!?˜´¸Î™Ûð?›‰êèå"D?'ÎŽ¦˜»w?¡z<ÌkO?'NÄ(H"?ï^´;Ðî.?š_)åL?rüý.µÜ?\¤írO?ŽÔë
-Í?'wn˜:P23FGL J1849.2+6705@X_[íöé@9
` ÒŸÀ7¼0íޕLÀ;)ÆΆ
q?øÖ)vò@8t1Bî@ðwy‰-ç¿Þã)ß]¯¿ä Ì=R=\¿ä]ŽGoÄù¿æàS*°"íAGNFSRQ?ïô£ã®Ó?Tâzn^öÚ?LÓA
-|»?LeMâĞ¢?C/d8?JH+«"?ïÕçÒ¶;.?|ā#?^&È=ÄË?c²‰ˆl
Ö?kÉ*ýîZ?x‡Å äC?î½Pä~Å?–ÖµpMÃ7?•êøÏʦ?'aK§Œ*o?'k"U\¶?Šbnl í?ïý_é=2;?Dϳç~d%>Ò¬-wšÎ>öÝŠƒ¢?4¶`Ž?DÅÏgW´Z3FGL J1849.3-1645@1³q¿_üÀÀmœ@ÔÀ9Ö®8HÀ;=Øwûº ?çºõ¬¿ç@
~ Lf?ù°ŠŸ*Ó?åUc¬En¿ï÷Š9™­?ïÿ}'Gÿ"¿Ú	ÞxúE_AGNbcu?êwÖ6èxš?Ä']
—'{?Sºªïu:?\ËL¶x?Åú•¯>®?Äv5p¿É?éÇ #È?ÐfÇÕ¢Ý?'ØwE"}?¿ÿ",ü?ƈpšÃ
9?β¼}àÞ ?ëÐ0*b*æ?§ äøŸŽ?™Q˜)š«"?ˆ<ˆ€¢x?»*¢‡ýæ?¥O¬š/ܒ?êXb>œ¿,?Æ|¯+sõ?U£wUSNú?zºù2H}?Æs0â\³?Æ}½×Q'–3FGL J1849.4-0057@?Úý¿³ß–?TÜà‹À7½ð÷3©À9¾Ç¦^Û?ø»òː7@y'W'c?ù'cð?m©?ï	Bi1¿Íƒ'[·¶»¿ãµ3S£K¿â¯ò6á"OTHERsnr?|²Ö»?{ )å€÷"?³Òp#$¬?¹BÌ£ýo?íLMàûïL?º¹µñ+?ˆ;
àêÅ¥?£wºd°HU?ǐ°0ßL?ÅC6Ûq)?éºç¼Dè?ÆgÆ~9E'?®ÓÂÚPr?œžÌÖÀ'?ĺ¢Ù\""?¬ÈYTq?èïê
{5Ô?±lc)þý? õøtM?žôÔ6•?Éò=Æw9I?»–÷Âë
¥?ètjïÚ?¾­Ùn×3FGL J1849.4-4312@vx@À1Ú3çüÔÀ9C΋é®À;UÏ2e®?꬝ØB¢@ê#3
ïG@"›€y
¿Ñ¨õRäÄ¿á9£ª¥}¿áҜH[ʒ¿æ—þ7d+ŠAGNbll?ﯻ®ùÎ?zù†…üíM?e¦‡5Ö·?d<¢ÖÑ?}Nå\-þ?u¿ÄY_ß.?I3?¬>†eªr?‰Tôˆ?‰bÙaÊ«­?¡ "ç'Þâ?¨quRIA?îVÙ¾×h?™ïk£L–?™Áuœ7?ŒJ F"x^?¢™×Ԋ;f?'ÕÄ9~y?êÃö¬äïÉ?£-÷"7xm?›€ÃÜ?ŒÛ?ºšv?Á€":Sà?¢àZ¶Š ®3FGL J1849.5+2751@LøÌ?ß @)a ˆ5ÄÀ9µ§íÀ;~¬ 7?ñ5†oE],@ãîƒ*í?@¨8ßðk
?Á—'ӝeE¿äši¿ê!Û®"N¿ë.¿±qAGNbll?¹n‰æKÒ?´éoŽyŽ½?êúÞ¨öZ?¼ÚÚQ
?®4夺?¯föÙ%?Þ<Ô«T?ËoçGȍ?Óð–ÚWÅ?ÅÊÕÐFš?˦£ïùÎ?ÄQ+Iwû?àëJ¼™b'?º¹Ã¼	©V?ÖAfÝ3:ø?¸Kø7SX?¿ ¦gÿ•?¢4‹¡y‰?Ôµ	âÿ¬Å?´Š˜†öÒ|?à
rJ!7x?»½µ'ÃÜ?Æ`#{Ȗ?²Êù‹7†3FGL J1852.4+4856@S¦ó?þÑ@3õà_PÈÀ8†oÔ¤1£À;Œ.î¿¿ë$ồ¶Î@˜qB7ˆ@|yÿËQÍ¿â?J«k‡¿å¯uˆ8¿ã‡fýŸ¿á¤mÇr‰¤AGNfsrq?ïúþc«…Û?K@#Eó(?Ž³†v?LˆL#?AT¯[w¿I?Jšw<øÝ?ïÎß4÷lˆ?õìͧ{a?\":+
?bŸ4•*Á?q‡â½;1¯?€=@ß~‰Ý?ï!ŒØ…é?Iôñµ˜i?v+únâ½?o¶ÜB;§ô?–Cfb6¿L?‹Î8§p:?ïùk"?SÃ<I~È>Èø.ƒ >áPÞÆé‹?J9"Äu5?S½|˜…Àn3FGL J1853.2+0006@@€ŸÍA¿Ö!Ÿ¯T¹À7¨R$AÀ9í
ÒÁÙT?þ™ ÍÕá@56B²,@6L,ÔIn¿ápòÁ~%¿çr(+mA!¿êˆyê/g¿ã­_cŠ5pPSRpsr?náãí"r?tB3ú/ï?¯0NQ˜ƒ?¶³SŠ¡Ú?íï»Ü6øô?¶·£/Öù?j†,Üb©u?{r
˜)Í?ÁŠïçÃÚ~?¹å f>y"?낽Ù2¦¸?º5îm6o?¯xËèvl^?à¾yžÌB?Ätgþô }?¬—"Pãö?èëYA»'?°;ÝM¼?w
oÊ?™H¨Ï=Ž?Ʌ{¬?–Ó1¤™?è²%ƒV«×?‰S(€wM3FGL J1855.1-6008@tþí )À7½F@V1eÀ:Îç·3ÞTÀ;úŒ3‰M?çv1Npj:@›Â[YÂê?ý'(º3?îÀšdoÁ¿ÔÜ	
•°+¿ÂÜú.&Pn¿ß
ZO4y7AGNbcu?ïï7EUí?[ù²º"';?N¡ë±ñ¸"?Tk¤¬%Y¨?R@{-I?QÀùWoù?îx酝ք?­Õ²´èn?½¦œÛ!…?""Œ‰:la?¡ýþëÏl?¥qÝâÞøq?î‰_Ço#—?œ}>[@?'"$Ìz.?"F¼²|ï‹?œ?âE¡_?…~-ñfL?ìtgUÅ8?°ž\?š™?™¡|ߣ»v?¡Cù1\H?µ÷hçc?ª0œ¡ 3FGL J1855.1-2243@)½«ÓÚÞÀ%ÙHßlâÀ:IR}ÔAÀ;ˆÙÔLg?ðÖ{<6g@.ÝTYs?ý"ÔÁ7î.¿áøK€±ì!?é€à¶cª¿»-""Ñ¿ä¥wžG(^OTHERglc?ï[}("‡§?˜ßº¢Š?}SmÇç`w?†Ÿ‡Lÿ«?Švþöêfl?"Òݞ;²?辤®0ã.?ÍßV^:û?²çÀ›
3?¹~sÙ<Šþ?ýyfîî0?Æí5I,•®?ëͬÐ?©¹'§Ì+?±Xá+җ? ˆá«Bh ?°:=ó>í?÷œüXˆ?ìÉ|9þ
?´˜¤‰ß[R?²E±ÈåA™?²Út5–õ
?¹±œª8"?Ÿ'åE/	3FGL J1855.9+0121e@AS°
kù¿ØÙ"`}ZÀ5XôÀ0ÝÀ92ÛŸ'@¬	íI@Ö|O[ÝÌ?üNoVÏðn¿Á~õÔX¿â*ªcy¿æ;êý9|#¿ëvO²ÅºŠOTHERSNR?¦·¼ô$6?¤?ÜçÁ?é¼,é|ã?ˤ°ÓÃÆ·?ÅZud'‡é?ʛÕÄaC?"VBŽV]À?°¯™6ͽ?ç|æí¶!?Ë¢z‹
úü?Ðe±àÑ?ʘӤcôð?¦ÿkåžr?¡)ÍE
À?â	¾sÞÅñ?¾Å÷žˆ$'?Ù•›Ÿ`O?½f(ȦzÇ?]–®Û*?^ÞÇNð§?á¡oí&6?ÄòBtا?ܟ"ɏ·?ÄïF4¢4ƒ3FGL J1858.2-2215@+5}¡ŽÝÀ&»Ú@RÖgÀ9'Τ=aŠÀ;‹½÷FóÚ?ý…'MJ@C±Û"Ì?ð³!Ø?ËwúzQ¿ÂŽúPµò¿ç·f'¸¿í˖ìÁôPSRPSR?rðü>Äjí?vKªð0ØK?îQs­€½?´D48JØs?¨'‰=OfÏ?³Ìiž2«V?£+ÈM¦õæ?°5ÆÉ=É?åµ¾<è¡R?Ë\2ڏµ?Ò/
|yÞ¡?Ê@'Á+*
?¡TÛ­€k?÷B-yý?ë´Wr"Qø?©oÃkQÖÆ?¹³}Ž°	?¥Èɖ…ª?ÀœÊ&OŸ™?«€ýÙK&z?éúbä³w?µ¹2k—µÚ?µþ˜œ;%?¬Å¬›óJô3FGL J1858.4-2509@%ׄABÀoÀ)8!4x®À8Ý-?~À;7é;˜\ƒ?ðÓDá"@¸vb\ìj@Lú¿¤ED¿Ès˜•¯÷v¿èÇON6¿àYÖú¼ãå¿ï	Aš:eAGNbcu?ïrÕЗ¾Ú?›û'ïÚ%?€=€IŸJÙ?€²bh	Ց?ƒ
pþƒ?…zæƒinð?îXC—Òÿ?­Öø€&—?–´k¶B9?'?åe(ü?£tE?¥?©(]´Þ?éò+?®¬C?­M¦?À´uÄÔ?¦®-¦¤!A?¶‡†ÇÆn?¢^ÓyDSô?ê‹:¤à?¬Õ¹0";?Ÿ"Ì(JT©?"Wj.\D	?Áà|vÈ!ê?«gKÊz3FGL J1902.0-5107@u™ûoÀ6c
?ƒ£ŽÀ8}ík¨ÆÀ;{,Ü×ÜË?ýR=›¥@T˜"#@Ä Wì%¿Ð!°¡?w²¿äPàɪ·¿åÇh>Â*¿î9uýˆ+ˆPSRPSR?–<ÛˆÜï?™(dM›6î?îáXT";?¥<øÇ@?‹04׍7o?–AõàšÚ"?•iꮯTC?¢m
•ßò?ëîR?/í?»Þî5¡Ýu?»2óZÔ½?·<sÕbø?¾\Q膅F?©¢èÙ-Ç?èÓVÊÄ0R?°^¤Øæ‰?»÷ÁWø*?¢Oòª'ûù?©mÍ)©	?œ¬©[È?ì	Y'Ø1?¬,Þ€¶'?²þt	\iò?¦×PªÙ¶S3FGL J1902.9-6745@t} FÇeÀ:
%@+i:À9~s£eË6À;¾ç!â¨×?à8u_ÜA@Ü¢­¿ke@ÄÛ Ú+¿ãzƒC8[^¿ë:Û}ó)¿å9ËP©nV¿âógŽ¸ÅAGNfsrq?ïö7öi–3?[̋l¬CÏ?+i^N.?T÷?´?P.	Ù?RT!Bõ¶?ïÀq^ϙÈ?{ó×Åi·Î?Ur÷‹ÜH?]>
ÚÀ^¿?z†óÚP%f?xRпƒe™?ï¶^É?Œ­¡IÒËð?ºóŠ£?xšÉÀ
³Ö?—úwx:å³?ˆõ
}Âbs?ï¸%o+"É?€;«Þýê-?2­gš÷j?9©>iÈÞ?a8øCT‡?ÿƒ;[3FGL J1903.2+5541@U~¤?åÉ@4‡ŸŸm1À7ÿ®õKqÀ:Ë>³™õà?ôźߺeA@¡Æ¹¸H?÷_~«+½H¿ÙžRÌ£¿ÕŸ=X® ¿Ú´!!sÿ¿á\äÓºãÒAGNbll?îùÞ·‡í?ªìdÿZ?pŠƒhO?˜ÎÖ"ïú?œ¡ˆ4þ<)?©[¡¤ê[ë?î#™Ž<ì¸?°û¸àIKÄ? Å~JÏ¡t?¡ô*zԙ?šÑ¢Ã& ?¦5S	ó2?鶏ԸC?°ßXtZ³–?²c…ÿÿ««?¢8Å3?¿çûZ?ª<?«1œàIÍ?å ÂШÉ?µóHŸluS?®Îè 4
?§Òsû¼¢R?ÑêáfX,Ê?´•°fii3FGL J1903.6-7052@tEõŸôýmÀ:'ë ÍjÀ9"=çÂÀ;¤®Zþ‰?å8æg—Wº@¤ý)+@‰mèþ‡¿çxû@Ÿú©¿Þ*Y©ÙF¿å50ûdS«¿í˜™ç2«PSRPSR?áèÓÕȓ4?ÉAº:)éq?Ø°MgÌ?Èêúûõ>Þ?«îIÉŽ_?¨EÛòßp?àeíÝd{‰?ɱZfÏé"?Ñ
»¬]j?ÅBÖîìþ?Ì@3W?¿¡)UoÈ?åžáG
·?´Ï·¯|£Á?Ì_*:áš?±½À*1'?ºQœ›Ï?¡í‰…"?â«(ÅVª¨?½ùGðº›?Ð5ø™ÁÎ#?º¦OãÀc>?Äçk·!¹?±š¢Á$M3FGL J1904.5+3627@PÕlÿݛQ@*˜Ý ·0À:HŒŠ½À;»©°h8?)z?¾´?@
*)Ö=8ñ@ÉXŸÿ9\¿ïÿó´ÿH?ïþIãñ#¿âޔ`}Kä¿ÛýëJDAGNbcu?ïÁ<Ú䀲?€­•½`®?TS¿ê]¾µ?U²ífÜÂ?zL¢"(7
?~:
¦ë
?íÔ]¢C,?¸¼NwÖÂ?™_€Q¢|1?¬Äç
·?¦ùý
$?°þ…%Š?î–U{ñTÔ?"*^=!¬?Š[OǨô?y€:Ñs? ÔOuÆ?Åõi5à?ìù‰lrÖ,?²âɄxB!?²ùÿX5
\?±™H@[N6?"æÕÑ?–°0õiíþ3FGL J1907.9+0602@DúÀ%¿ìÔT@(4À5ݜ©'žÀ9êXR§lÁ@.[ê¡õ@ÿI@eË·@$̦·9¿Û²oË·Es¿ãfCo°+¿å‰¥ì@ãþ¿ìëè%óôPSRPSR?=€8 å'ó?Cùý	æÑ?ï
/|ÓÓù?«êAo¯+¹?ä…êâ?«¹ÂºËÎh?<šO×Lo?i¾Qé?íÖÆ@+?·ã݁ÂŖ?·\¯€>'[?·í¹^Ü_§?˜ºÒ<½DË?"¡¨^Ë*4?ç«cýéFõ?·Èk{ÞX?Î;ÀÃ;'?µå
à[ö?HÉ‹I"[?Jñp«ä'?íV…M?«R°‡"\?µAb¨ò?«*˜n(ãÊ3FGL J1908.8-0130@@ÇûÆnåÀ9±êFÀ9ªð]ˍ2À;²g†÷Öf?øçj@
ÌiûqOù¿ëyÖ1iH]¿ïqªôy¨Ò?íåO[¿æöË,¨nb¿í™\ZHö¿AGNbcu?q¢F?"Œ»?†š˜\·®¨?î9eÄð‡>?·Ú".·B‹?ª5Zéú~?¶ä¼™Â?¬å]1C@?²£rnð5Ž?çZ:NJ-›?Ó@µÆ"%Õ?Ð^#F°?ÒÎÃÕ8yÓ?¼×»¢,0Ü?¥€xÿÆðò?çØ's»?±³KÁÚºe?Â3…Òœ¨?ª¸t ZU?²Q¼ÑՅp?½	ÌN‹?덬mP«?ÈlxcÏ<ê?±@ßÅWõ9?ÀõTȤJ3FGL J1910.7-6000@u"§e4À9žÚà‹ÆrÀ9ÚïÅYbÀ;Æ{…²\?ô£D",î@ÄáÖõÈ@š½ …«¿ä»Û®ã¿Ù·°ÛÕ~L¿çæ"gÞá¿í»ûÄ1OTHERglc?¢ ¹8+? ·¤( +?íøŒa(`*?±îÿ±?œä3¯Šg?¬Å|k'ª?Ò¸Ò´GÖ?Åpå1,%·?á¾MHv?Èo.kœ]?Æ?abN?»…Â(Ãoß?Ô¨—aC~¬?µöÛÊZ|Ÿ?ááQí+?·¶m"Ù§y?¾TñØb›ú?¤îoO¨ã?Õ¶í·Ã)-?µ»n2NS0?âŠDý¸Ñ?¹DNƒ‡¼˜?¸¯öù"Ä?¨+͵Æ-3FGL J1910.8+2855@N{À?ö@!ƵÜê&À:8ðvö£À;€d%C†h?é{noc)	@
~†ܖ?÷jŸÁ%ú¿çZÝ÷lˆ"?ïÿª,cä¿Ùd¸&'B¿²¸oÕrZ2AGNbcu?‰¢[?'Cˆó=‹ó?[1¶R?a;(³IŸ?†ò=€ž÷n?'pùpÇHÂ?î}Ïc×äˆ?­Kzæ'>þ?1í0™µý?†ÿZ	VÍ?£ÖŽv[J?ªj/]$ ?íÎ|	u¥?ŸòŒ"Ûî²?•Ùð
#?ŠõuƒaE?¨28¢?š¡' êÙ?î7Öîž
?¦K§ïlÔ¡?œ¹pmw*?¡JÙsV?œKÎҾǞ?›¶æ×c3FGL J1910.9+0906@E ßÔŽ¿ÃäH~ôÒ¥À6k3æÉÎÀ9–M$v?ú´'ÇÅ&@¡NÇѐ?ÿk"Æ(˜Ð¿ßc%  ¿ä\áýál¿àUf.2Br¿æ´7À
DŽOTHERsnr?VRX ‰â?T{ˆæ÷«?‰y…¾;F?Œävð}¹E?ïŽðÜX¶Î?Žt'mÁÑ?J€spÙR?c»¨H?ÑVþúÆtN?ÅueÁWu*?çMà{é£?Ńئªý?®Âww9YŸ?šð¾rGÒ?¿‹ö‰Cp?¦­]÷¨Ÿ?ê"Y·cüb?«UI½?}51ÄÑJ?]óªbÊ?Á´:"}?²ˆcã%Gò?ë=Þ%ªKœ?´IžqåS|3FGL J1911.2-2006@0â
_ÕR­À*sç_JHÀ7ºÚ4"\À;Êʔ
i?óusºaæ$@´›Ü¿ß@E¸7~¿ä_Œ+Hk¿å¯rÎ"`¿æԃâu¿ê]8ÉÛxAGNfsrq?ïÅ[Φ.ð?u´èF2õ=?lrGïu:?oñ;I§Â?n1éjϛå?kZ4ïÏ?ïÄôïÍÑ?÷ÕgB]?Sz^¼6`À?ZI‹ôhÓ?x¦ðÐ9?|ljTV\ñ?íQdø^J?¢…6åø+?¢q$8aC?•ÑÇ7?¨x™è_º?™˜£Eû?ï¼Òf?ÌÖø1"Ä?6ÖP<³?D-
Á'®k?€
Ç$i?…î?3FGL J1911.4-1908@1ÑŸ>õÀ)½ôafLeÀ9j+Q½aöÀ;6dE#ö?£7.aߐk@"î´þúÇ?üQ¦áUÅÚ?ïµF2`Ǹ¿Úá–|y<¿ÒèÛµ ®¿ÖŠÛÞ$AGNbcu?ïâî–3°?p%ö*œ?F¶k´.C*?F`š(¯ud?gcÏÀ¿_?m¾_w>¢?Lo'Þ?•È¶©J×ô?cUL"Ú±?f•½üB?†;+úQÓ?"+¨ÁsgÓ?î@ÞËÃi?—f¤7És¥?'N³êS?'<}:Ž?£KuíÔ@?"›·ÁÐ\?ìғí½Àî?¤ï íïÀ?[H­×ÿ?^à‡uW˜§?¸ý#oZœ0?¤ÂSÿæ¸g3FGL J1912.0-0804@<	I`œ"
À }ÖOÀ9~ø&²òÀ;Œ#QA¿É¬v|DZ@Z¼#jR@\"Ý¿ëÂÏÏÐQ+¿ÔÎ)¦cú¿ßrצQ'¿éú–«õßAGNbcu?ïø°˜Õ?ëÊ!˜_?€V>Zah?…ŠÑ'ÌÄ?wd×*þÓ2?|‡c+úÐ?î™aÇáF?¬'¼'M¥?sªWtgùf?z¾œxW·â?£ò¾ôôì~?©ÀRŸ¤X?ìµxRƒÀþ?¦Çmß°ç?ªjñѶê2?žØÈãk²½?ª=‰
ç?šBÒ\ad?î
ûò;1?¡ù­vH‡?_¯Øáž?ZàÇÞ=J!?®RÂ/æí? ¸òMNsÈ3FGL J1912.6-1223@8+OP À$‰®ÁIÀ8Ú7æ÷~À;!•ÄøÿÓë!Ùf¹@¹ø`Nt@ïÜÀŠÊ¿çƒÌZáøÙ¿æÃqù[dï¿ä8,ŸÎÅ¿âñn±}UAGNbcu?ïäãO_ö?j
{-ƒþ8?/s$V¦?1¬¸rØÆ?i%~þ:ž°?iV‡±ŸÔà?ïÔWpq?£ã"8ºÿ9?hÄT.±4?t¤QYʑ,?šê—À?¢é?Ÿ?îçÅþ?"²SÐy Ù?ŠLȈá—?~;ÅhÖ/d?¡N‡[ñg¯?•í°Æ?î'åèŠÅ©?Ámþâñ?D*P~Wq?EwÇ4̇ž?¦ø5ZG8?ƒÜ¥Xï	3FGL J1912.9-8008@s <€"ÞÀ;c¿ÂùÀ8²gˆ¥UÀ;CE?¥1}?÷õýR{¢ä@ÿÿL%óZ@il(¶X¿àøm"—ø¿âøëÒݙ4¿æ€;WM¿êŸ½¨ %AGNfsrq?ï¹Eßþ£?|®¹Ïºþ€?t´>-¯SA?wŠsä̂6?mQ¤‰¢¶Ã?lÅñIŽÝö?ï«Û[}ÉU?'¬¿A'h†?\ç'&tŽ§?c]ðº	.?l6Û¿´?­z/§n?ëýâ°'?¨´'y1ßþ?µm$3tš1?¢¹WÎÎó?­çzëÉH?›ŽçA"d‡?ïu
P†á­?Žþ¬Nª›?]6¦f
x?s•Òª ?%	zÒÊ?Œ8ÁÌA3FGL J1913.0+0910@EÇwàmò¿â:þ Œ=À7éç3ö¨À9ʜcxu]?ý"T¦uu"@
Eq•n'®?ýiš¨¸E?ïÿf#dLõ¿àñfœí1¿éíM¦¯ŠO¿înÂÛ(ÒPSRPSRP?+ r4ðè?0>ó\!?ç$«5}'z?ÑK¤¸{+a?ѳ5†¾<ñ?ÑJ­	QË?*šÅ­è"Ì?RõõZ?ã«t»‰NS?Íwû½€|?Ø¥Ã07¦G?Í­¶÷œ?‰ÙO/ðsV?'½	š†—?âX7º-`?½ŠŸ1!5?ڀÆ&y¥?½aßùN?lu'Ü׏'?mZñÑFv?áôfˆ/>
?ÇUçïj?ÛÞGéçÔÏ?Ç	&D֟3FGL J1913.5-3631?óA« §UÀ3å*?nªÙÀ9·ä$gÀ;qBÖ>f?؟ºoýéÐ@lôÂ4B}@K^ tT;¿ØÎÖ1¥i‡¿åNGÉö·5¿ãaà·);Q¿ãÜQFAGNbcu?ïøû#&#)?CÞ,•5D/?Jr8L?&}‡"ÝO?Hqj,]W?AÅ%òˆŸ?ïÅà}Pº?|	¥¥þŠÅ?T€É×± O?YìG©BQ?wïŽâ;D?x×Q¹V9£?ïêK÷õº?…p"ŠiUî?'ïÔšŸ?uøȸÑ?'ÊÌv4Fk?a#0º?È?ïÛä½{?ol¶GßÏ°?×}‹oø?©QƒÙ¾?qßáF¦+¯?o4í³Èh3FGL J1913.9+4441@Rö+`Ø@-÷™ÿðæˆÀ9úâénÄÀ;ª
ájÃ?Ü<<
Lo@F¯ÀÍe#?ýužèó¿å07õËÛ¿ÔúòàæN¿ÔÔߜC~@¿Óž£:†§AGNbcu?ï¡4ìN?›èqjÜ
{?Z cæH®L?fAØØь?"k²µûÖ®?›yiR˜ H?îtƒ–å²?¯VR=Ì¢Y?Š:Do­Õ¦?ÄY–•å?¢)5u¹h¿?«Ló6ݦ?îáåÚÔtì?Œy¬GÃ?ˆs<,öŽ?z"¹a¥Z?—ÁZç,?†:l0Ðà@?íˆÇN Gu?¢¨Ǟ¶?‡yúY¾f?"&Š¥
V?°Ê¥o²Œ†?¡%Șe#3FGL J1915.9+1112@FÙIàâi¿Ñ._ܒÀ7ý:8
2‰À:;i…Õ—w?üÐ=‡Êå@‡žT"Vå@6ßïiYá¿á­å_—¿æÄ
¡C²¿è>ÓåÅ¿ïþ—ëC°YOTHERspp?o"jÛØB?q›g?!–B?Óƨ€C
å?Ïóná'­À?åý'Ut5?ÐÅܔŸW?"/ƒ"Þ3?2Wˆ¼s4ƒ?å .©.'?ÄRË&às?Õð
µj­?ÄR&Ã	˜?±Œ–)A
? ·Ð½mqW?Ûç7m7?ºÈÞ…4?ßµJ>.ø¬?»Ç¶ˆæð?Šþ3Ÿ'6?w×iXÎ?ãYTίø§?ºØ
PˆË?Ø|†q?»|7·Æ3FGL J1917.7-1921@2<‡`±ñÀ,§Úáb†À8'Yáó¥À:Îÿ€¾?ãÊåÁæ?@'"T±I?ýòÓÿñè:¿É¨còÿ͑¿ÜøÉkI¥¿ÝF*ú¿ÚÙ©Ê>R AGNbll?ïj]îT՜?'nß(…?Q¯áh³'?UéÀóãen?'£Ç7NÁO?ûƒcì?ïi-."±?˜؞íu±?m5b0û)?n¦¡z­2w?ŽmÜ(vœ?–S‡Ëÿßú?êàjX~?¯\¿D
#6?šøçX$`?…'£ná?Á<‡;™|?¬ÿ'y¯æ?é)zHdž?ªVü&8çÉ?{îפ=?|½ü®W_g?ʁPL%c?©÷X]^ï"3FGL J1918.0+3750@Qqb¿è¸¼@&äÔßÀÅXÀ:jå€!ùOÀ;ÅÃqÚ7ï¿ûŠ­ Œ§ï@j£¼2K@‰_²?¿å_Á¤$·ð¿ãÞOªüÝ%¿Ø¡=6÷ì¿ã«ìE@¯{AGNbcu?ïÅå¢ú?!u‡ˆ¡ƒ?<†Õh'e?>;H?{EØrÝ4?~¥Û%?íÈ7øPG?·oÂ…?{"¨×‹Ìj?‡ò·¥ßi?°üšÄÀú?¶<è5Ó<Œ?îè%@<@?™·æ]ý ?ŽQí¸ÚE?*¡!ÑU?¦}=öE€?"öÿßW?ïf9A|w?‡ŸöHÐ6Ø?%¤¤sâ?/šÔ£*ŸÊ?"
³4Iú?‡Š¬Omv¶3FGL J1918.2-4110@vL» 1ίÀ6=QÀ¼ôÀ8ŽÄ¾áQ¿À;E%£þw?ù®:m$¡@Àn&nª?òÕ5 É#J¿à;Y2~àä¿Èì0g"/¿ÙÖwø×d"¿äü/Ö(ãpAGNbll?äôˆ(\ý?˨(÷–Fg?¨3µÖìL?­¡fèPÀ?Óxôh|f?ËXG0ÿ ®?æé«'è‰?ÈÈûž7'?ÅbK	?Áý'Õb|?ÀÓñ"T]?¹ç0-ý?áeƒ(Ó´s?µGÛâùûö?ÌÄÁÀ æ—?²{OMè\ð?Í¥1œGœ?°Úy0óÔ¸?à÷ã7ÁšH?½7Žõ	n?ÀœY'®±?µM¡òÿØ?ÕÂлt?½i¦rN3FGL J1921.2+0136@B㭟àÛxÀ‰¦ ¿çÀ8Ý^ʐ²À:û( °z?à÷èόš@…#Ôñ^}@º 3§!¿çg.ÀæBG¿Ø¿›¾Ycì¿ä`U£ª?¿í!5ÜI±>PSRpsr?Àöd0?»õ8?âGë5w$"?͍2ësÑï?Òõ!ߟ¹?ËG|YyO–?´Íy'Ù^?¶zS#ÿÂ?Ú³™ÇèÝ_?ÇÙ–þ§?à%lÙV%?ÆÍØCöøs?ÖhGÆæÆ¥?»'aü.ì?Ð"¢ƒ;ö€?±¹ÒYµý?ÙuµÝBÛ?ÀG=­p?Ï>ßôçóù?²Ô™c]´?֙»4m¸ß?Àñ­½-?ÙÆÔÑM$?¾3m±w£'3FGL J1921.2-1232@8ô¢€Èè<À(u¡ueÀ98äŒÜòµÀ;A_~Ù?ᓧº[(@b~Ù$@Ihßg"?ìíbM@êE¿á-V>>ï¿â2Çc½{¿ßڈíÇCAGNbll?îW©ç
×Z?©H2oNÌ?ˆlX¿Ç?ˆû~øÁg?¤exòÈ1?¦Ûª•QÉL?çªPΚXØ?̜®ZòÉN?¸?óúR?¸}<Žs½¡?Å6ÃA™s™?Ä«Õ¸@9"?ë·äº+?¤|®üVÎ?¨(¼>Îè?"BmJÁ0Q?¶7ä|7*?Ÿí—NýÄ?Übl˜_rk?ÀÒêåù€_?À©€}Tñ?¶‡pã>¡?ÛHÓ(ö	?ÁÁlâU3FGL J1921.9-1607@5´ß¿ØÀ+Èô^â
§À8ý»V'ÄÀ:òéû±¼¦?仍_Ø
v@V;mê>M?ùØÏY§f?欄ñì†?ËA~ÂRË¿Ø	žBI¿ÏjØïx{ðAGNbll?ïo½?›Í~ñ'á¤?W€Ñ-ø9?_u'€@:E?¥ëFœ?›Oa¬ƒ4?ïz䮙¡?–âõ4!Ï?iVv™bQÑ?rµ?f¶?Šñ6³?+?"А9¥ÔÒ?뚯É+èg?«¨¬6ÀK^?ŸX¥%dÔ×?'ÐY}`?»TXmG‡œ?¨•'!LÀ?ë±¥­Õ?²KöȤ?Œ5L!ü?Šò¥®ÄÓ*?Â5⤧(é?²Õ¶4Rö3FGL J1923.2+1408e@HŽá@!X?¿ÝŽ™¿óå.À5É'm,SÀ9'Óˆ¨°Ž?ÿdF0eùY@ñÔÌËu4?þ«äÐ(Í¿Ø3)˜—¿âÏ^w"›Ü¿âÐ¥Õ>í¿ä®ÀýᗵOTHERSNR?p¤Ë'£?k¶"ÿy*<?'×>·>¶X?ŸkãÂ?îu?ïHæüsý? kÒ£]öa?IñN2Lßõ?bÝð2…ï?Ñø3a´]¿?ÇãA]Ɂ?æýiû™=è?Çèiˆï$~?ªIžrŒ¿? 0Ä@΋?»=†í¦?§R0½˜{?êö³µX™€?®—ÕV‹n?@=SV'4?ˆqdzÜ#?ÍT\+u??¼(3Ÿ/†Q?è5çÿÕWœ?¼XB#³3FGL J1923.5-2104@1.¸À¦MÝÀ0A'ÿùJÀ7û:Þ"_¦À;1!àûX?ýÎrn²eB@EÍNY?þ6¾¾P¤¿Ø'#_3¿áñ"þÏÿ1¿äay¯XŒ¿ìÒÖ{™ ÈAGNfsrq?íˆõ‡B<?´þÚ+£??±)%fäÙ®?´ô‡ßmÎù?"¶Wg£y?ƒ3rý<Àu?ïÂôòÅÃÃ?ëNüD?V)µCSQ¾?[iOYúó?xûLII¤?{Z§"P'?á±°vN¤?²ïs':
?ÓÔ%¢?±¥@2º/µ?Á'%ہÔn?¨[t?˜×7?ïßæ^s¥L?v$¢6åß?$£®_°"'?B1VÍ*®ª?nÏf¦_ªæ?uԛ¾Ì¯3FGL J1924.8-2914@"´ö€$}ŽÀ3œ`ÔV.À8+¨¶mÀ;@)8Þmß?Ó÷#óC@0ƒ¼7©:@F¿×ñÄ¿äVÇâØ'¿æ^òŖû¿ç¶1<¸íó¿å-«eã£mAGNfsrq?ïõRˆ"Ä>?e¹1u؂?<&²g@?J+ë±x?L«L»3.?c—Íçlñ?ï»II?ëE|R´?UxU˜@Ü?[mYó
mt?|âFh$u?€™''a?î̕¬½6?—Ž¾Óٞ?†>¡ði?~ª¥ñ:ïÆ?›N!p$Ñ?Š&U´?ïŽõQí/,?‰Á\ª*6·?3Gn¯?<f~.œp6?‹©¾šxÄ×?‰˜-E»/Ë3FGL J1924.9+2817@N篟•\@kDß­úûÀ:p3SêÀ;~ۋ¬q
¿ãP¸t{'@DÖ(–!?þ$º_ÿ¿ïÿûZÔ·Ó?ïÿ'IÏ_'¿Ý©ªFB¸¿Öt¶©R|ØAGNbcu?ïæòáø[B?hù ,*Ç"?@]yŽ9ƒ?>nX©Â«Ï?dõ¿¤q?fîìÃuU?AZNî?«Ü0VŠˆn?o½äF?yTu¨Ú¹?¤ ©?ª¶ÿ(TX?îšÍ%AVÑ?'׃°pq›?…f«mS»É?v¼&"‰«Z? ù'Е£ò?L%ƖG~?ï¸&÷‡%ƒ?º,ÛfqÆ?Z¸Ã<'HØ?_ߞßA6(?}>SmL¬3?€»«Ô5­3FGL J1925.7+1228@Gõ¥À‰d¿üw'áC§JÀ8'rϏÀ:lêÔЦ?à¨I¾B£ò@ëºùe²@Øó_ތé¿×W}ê*o"¿éÊhó‹Ë¿çF:*.î¿é.ð^ÞmðAGNbcu	?å˟¶ÙV·?ÉîJûº'¹?1šù2Ã?ž‰²·;?ҕ§¸¿d?ɜvÚ·Û×?܁/ú«z›?Ô­
×^Yd?¯×@›ú"?³MWû¼c?߃çñÕC?ÓÔV]Å?ÖÌ»£êw\?µõÉÇsÑ?Á¨A§ŒŽ?¨²"ke"g?à28 á/?¶f!f+‹†?â쐕?¾™õ7b¶?ˆê?"ëa6?¼°Zž¯À?ÛÔâ.ó?¾5\­ïø3FGL J1926.8+6154@WS*`%څ@3½¬ÿ§ëlÀ8ªlÞPÀ;6w†IZ½?ñB%)[.@Ó;.ª7w?ýÓÁ`]ö¿Õ2¬inÈN¿Û;¿¦@Œ¿Ü4…²uÍ¿Ô¥R?=¾AGNbll?ïõqd/áÐ?TÀCiAf²?B*}¼¼?GŽ#–ì«Ï?H7D¼¢?JdÕڝþ˜?ï¦Aš±¯é?"YÿºMñ?q×Ø®·?p·ŒmS~?{ÉZÎyð¾?€-6$Áò?îŶþ¶?Ÿ?ž.y-?™ŒØ|±k?'Evºô?¢8`wŠí?"Ø•D˜0p?íù2ÕÛ£ö? °"D·C?|3Zß&õ?'óÁ ]¿Æ?¬æg`©ÛÂ?Ÿˆµ3n3FGL J1927.7+6118@W0€5D…@3mù³>†À9'&µvoÀ;€‡6À†m¿óؑÇ=@Ó@ÑÌf rý@#oÀbV¿ä=¾bb¿ä
ËHp夿åQ ¤®SC¿àÏ	ñy0AGNbll?ï݉Ý?ç?lÞ3(ÓP?QîLŒŽ?O0ŒÌ'Tñ?jPú
?j|ÛÛl4b?ï¶êY"L?Šfkø#á?f›1Ò ?j»±Ég<²?y=vÁ??‡®'hb{?ï
Ø& ›G?ŽJœ®a ?ƒúÕ#lê?{ÍÜ‹ôj?"Gš6Œ4?‡MU?ïteûÉU?ˆݍ¾O?4w؆ñØq?@M3aÞ?'+Þk?‡Á!&w­3FGL J1931.1+0937@GÍÀÓgÀ0î#;nÀ7þÍ;,&À:­?}ÄQ?É@-e²"@縨ã?ýà Éc·¿æœò1¾Ç"¿Ø?R}r¾Ü¿Ür£»Üdš¿ÖN—+™ûƒAGNbll?£{È_?'NÙ3ª¹Õ?DÅÀ˜°'?Fc†É%%K?ŠI{"íH?'69Õ	Ø?î¸ÉʇsE?«á
Bu*W?o´.Ç!¾?{TÄËÇ?¢x k¯Ð?ª#`ó¸íä?êT|¶›@ž?²>EE]Wá?›"
ôëx§?'`Mÿ]å?Ã;«fõŽt?°€Éá"\?îÝ ë•©X?Ýå;ïð?+–€°;3?3>gý;…?¢ZÅõ/]?É'}éý¾3FGL J1932.2+1916@KR ö½?¹†¿ÉÅaÀ7r?«ºbÀ:Rîu"Ó@‹1:Š•p@õi3JZA?ý"ò0±T¿Û ×æÜBŒ¿åÇÜÞÉ`¿êgž~¿íA‰Ï:ÿõPSRPSR?xóÂ\˜Î\?ƒˆÛ'Ì?܋pˆr?°?Ñ~}™š?áˆ`7
®‹?Ñu¥$°m?%â_÷|å?Q6û.©"?çk¸ßû?ŧ
uÒ?ÑàlBA)Ù?Ũd¡ôÈ?ž±"1á?"um«º~?à…W:Èô`?À	@"K£7?Ý
9G\!?Ài$ýí?fåæ´3?`²¼‹»Q?ë'ñ©?®Ö Ü\K?Ác4¡ÀÚ?®h¿äƽ3FGL J1932.6-4537@v
…@FA-À9ï)ªIëÀ9—*}'ÞÀ;©ôö·â¿ÜøbøGÏÍ@Wª³|D@ "À@øC¿Ú€²[Ìi¿ëbœ#P€æ¿ÔÑð֟çð¿ïÿí ²Û"AGNfsrq?ï͛îã8?'ì 7ü"?7"`+ÚQ
?Bœ^œ.q»?w¹Â‹¦O`?'yÅ>"?ïˆFS¶¶?‹þfZ;Œt?h7ÙôTÓ?nåMÀMû­?‡àt½N7?‡ðƒ(žbî?íÌ¿t÷ã
?œ~…6K©Þ?›_"Žg5y?¾¯ë¼?¥">iN4œ?–ʲ
4…?îꨳB{"?"I{¬Ó4?M±Lbx?K?Y·­1
¤†? Þ¯šNlâ?"
 ˜¯i3FGL J1933.4+0727@F4^ FÇeÀKËè À9Ìò''sãÀ;K®æ1ø¡À47ŸÔq1@"ôW€D‰?ûäÛߏG0¿ïÿöµÿF?ïÿ°²Ô˜¿Ì/'ŠÒÓ¿åSd¹AGNbcu?ïW—áqå?™ÛÐû·&?aZñÌG?au"VU#?'⛘C?˜õ`œÌ£¡?î´†üv??»
oFé•?}lîp(Ñö?•Ï<8x?«—Â3×?¹W÷8€§?íº³Ãïe?s@«"#2?"»Øáϒ¡?"–]âÀzÞ?ªv×RÝ@€?™VnÏôgC?ï­Ú…m¼×?Œ¥¿|‹?NjþC)e?xÏig»T?'¨ô¬—p?‡s/Kümþ3FGL J1935.5+8355@]ÁÁÖυ@9τ´Ñ.À:9‡aˆ±À<£mWò/¿öxƒ.ž#@"£]'­A@Çó?Ó)³¿èž	㉿à+xÿ›+¿çCú°¿âÚ)nä9PAGNbcu?ïöí×v»?˜¤ŠŸÓ"=?{îGñ*?'øîbK?uwÍ+±+?ìÔí=.?ï C8R2I?™$òí±·™?péAÃ÷?sLô+QÑ?~õ[•"äv?—Œ$Êá?î!™¥)¯…?›Y?× px?™´"5ß?'º€cWÙZ?¡d+šì¶?ŒÉЋ<í?ï¬ò«ÿ¶?~cÌÀWd?F{*9Á¯Ó?RËoƝā?ƒ[¢\vb?}<¿Ißò¿3FGL J1936.9-4719@uò®ŸðË°À;î€{»bÀ9he˜ºÀ;>`ñ—‡?Îí,öz'@Š+"+ÁO?úAÆa"Ú ¿êü¼Ëfµ?ƒPØ5¿2¿ÕÏ
ž¿ºhÿ{~Y*AGNbll?ïûˆÀ»T;?=j@¨.:?!ª¾é›&? c%Õ¥‹?:ë$ÅéYå?9­ƒ«´A?ïÄØ:%Ι?zpLҌ
?R/pc?TÙmè7Ê?yªWp?wé0‹†üÃ?ï)^}¸}b?ŠžÐ©àë¤?…ÒÑݺn?ç0åÕÊä?ÕŽ´&%ö?ß‰ÐÃ
?ïXÝÀ* ?‹Í.q= 8?50ì¯?Bð|–¡b2?"C³™øV?‹›MŠ7à™3FGL J1937.0-3956@vrìà2ÛÀ9SÂÀð À8ÖϦ›àœÀ;y°Øzù?à4èß
R@þÚæëÝ@fë¿VA«¿æ-Råf\ç¿éÆ@ÓH«¯¿çA#5åA¿éó¨—´AGNfsrq?ïè¥FNàN?¡5Œ:ƒU?V,M –ë?'º,5ødA?X‰%Á¡Í×?Íj>ü-?ïwzDóç~?Ž¯ìØÎ!…?jp'iÙ?k?¿¶Ÿ?‹ŸRžkàe?‹	I*ÊG?ï½ÕTø?ˆÁ¿ˆ+B?ƒµ~ÛFÛ?sÇgRÙ²>?–
|g½º?"ˆñ[‰Ô?îSRXjå[?ž–#+×Æ?uÌå^vka?pӁÛáÞ?¨=͂Üô?¾=þa3FGL J1939.6-4925@uÏ¿˜0äÀ;ÜLŸëÃ2À:5¢,RƒÀ;ŽŸ–2ÜÌ?éù·ê¬%@
Ý,µ?½Z?ùüÿ"µb¿î&µ´NÉ?ïþÖ¥œ9æ?žØh-Þ,¿äèòÂÕ¨AGNbcu?N¥B(?Ü›®ÊÐ?_À¨©a¢?bÕ4v'šç?"%¨¡šI‰?œ#}˜ë?ë f¼9"!?ÂÕÅИèH?±¸$0Þn…?¸
Ðð
è?µD¥íX€s?¶¡¯v´!?í'ÂÍâK¶?¡Ü(G5Óø?œ5Åt*Ã?'›°ÄµG†?¨ÈðgØ/??šÁ¯ý(i?ìaUÜó?´ÕäZ1‰Õ?¬ÕmlIÑ?®%?%ò÷•?­B¨_E?®E—{MU3FGL J1941.2-6210@tèWÿ›V2À=…êÀӚFÀ8´wM>w4À;xv̗?íõíqL@§[-M@%@u¿]MŽ¿Û[-3{׿æU™ªû0¿åIUÐRN"¿ì)Ø`Ô¬AGNbcu?ï攱øš|?bÜE¯3æ˜?\i[8æ?]-¬3m?V·2³¸Ïö?R›â9šÎ?ï¦-ëüd³?"\2sú[?[=·%¨×ç?b‰ñöˆÌz?ƒÎ1¸7?'"<ëh?ív—³žB? ar)9Òæ?¦œTÓ#ø?—tϝg5x?¡ú0ÁHº‰?'#zH!£º?ïL}n³úƒ?'x"d«Þ?`‡?'¡l[?`•š=vˆ?"_jDŒ'F?'ÇÄ;2›3FGL J1941.8+7218@ZÁ?ÐÐh@6ÀA¤À9]þÀdßÀ;Ÿö\OŽ?ó'-ªP@L÷¥¾k
@Z9¿¿H*¿ã•ó‹¿è"}š¬ál¿êISäŒ:¿ì–a\Ö¥AGNbcu?ï7â[;,Ð?™)ªÆ¹L?'XçXE?–gaXæ˼?z®uöÌ6L?|ëæî¢St?îuãÜ
?¡‡˜RÖ¯_?Ÿ'?S#É?˜F9ËNQ?'²`Å+<?'lP¤eô†?쳧ØFK§?§•ýL?±A¯z
þ?¡‰Z7'y?¢B#†)Œ?˜"Ÿ	Â&?éáwυ-Ý?°7öì¿D&?¾Ê,IˆÝÒ?«	Žh_vÏ?²*:M³N?§^gFB=73FGL J1942.7+1033@HÝ Y§;ÀuÈ@K·À8:Cû"~À:Á'h$¬ˆ?ïÃ|"jÞ@Š)åË?ý¦?Dc‡?¨lÑir¿ÒÛz,Êký¿ÝÍؚ$GÍ¿Ûܟ†K;ÆAGNbcu?æ
Ê·›ú?ĊËh©ùØ?—zKN5æ?"¡€?ÒrÅÛä­z?Ärüò7áë?çç<€*õ?É5-Ræ?©BfM?Ã?¨›<_hvã?Êt|"X>?ō"Çéw?å›Ï"u?µ¼ÄêvÀ¯?±MАdõ?š@Úpßâõ?ўt¤GÔÚ?´…qkâ%?àg‡$º—L?²Šº
<Å?®¢·ÇŒU–?¥?K
ƒˆ?Û\š½™F¶?³o0Ù>3FGL J1943.2-3510@ƒ/ÀÀ93_ý–™À9"ÞFqÔYÀ;‡^¼Mùˆ¿ÁˆÛrú?ï@b•ZDÅ@Â@+"-¿âÀ'Æ…z¿éèF>ÂwM¿â¸%ÔX¿ïÿʓ6©	AGNbll?íõYMœ5?­"e‡G>?f?á'"ƒÝ?hŸ5ª‰ƒF?¯FmÃgÀ?¬mEµåa?ìE­9t±Ó?¶N¾3»¬µ?¦'U†q'R?¦°UE¸¼,?²'kq!ÝÀ?®½;"'?랃¨^?¤Ã[{ôÞ?¬"'-Dãz?"Ðkn§!?´ÅèLž5?Ÿ"Aq›
?è¤ö‰Ãµ?°Þ1bF?¡ÛŒ« )?›y·q0ÿÆ?ÈøÈ®	?°.üÓû´3FGL J1944.1-4523@vAà?pXÀ;ڙ÷LÀ:²ÕíݾÀ;Åëõ‡:?Õ¾°>÷Œ"@
MYÁ<uÒ?øô­ÿ'+¿¿ïSZðç^?Är0ìSr:?¸
K?eè߿ڔcl®KAGNbcu?ïèm¶+?gÅ=''nI?4Þ Ûbõ?5:•‡I$?e3…Ôhj?f܅Súü?ï–cÇAa?ˆ'½ƒ¬ª?aͨuxû¨?gq¯Ì"ص?…óÏ°Ñhª?"³Bà£â?ï¤/œÑØ?‡´)¶` ?…uÆF"?|'¤À‹e=?"—	B{a?€‰¨CŒÐT?ïb» 0z?ð럥û§?HÅ0Ú<†V?UêLUM®ÿ?'ö¿(´?Ç*ߍL½3FGL J1945.9-3115@!Ø,àèÀ8"ªKÀ9-Ë)^žÀ;kÇc€À]
ÐXó@àqŸªÆ@̂Ÿ­¿æ¦;r®¿è¹áaÅ¿ØÕ5¿åÍæŽÙ¢AGNbll?ïF~‹Q?¡Tä¹X?k"µh™\?s"/:[q°?™ä­—ð'»? Is,*Â?ﲍæçÜ?…$Ò62Ìw?Xï€^8l´?e'ÃÍ)?€>–l~ûš?'Å° j?ìÌUëIØ\?£Τ…oÅ?šðÂLñà?ˆ‰ÔŸ§É|?²á tÅ?Ÿ›i"T4?ïNXßì?–]¸L?(+y"#?$ ô†~'a?§+&NEª?–[.ú'"3FGL J1949.0+1312@I«?ÚácÀŒ,ºËCÀ9²A'è|VÀ;A'¡ Ï?àäß@ƒå"¯‹@KxßdÔì?ïÿƒ¯]·Q¿ä7¯JA'ú¿æÌ°i·¿Öý¾Û%3AGNbcu?ïÄéýJõ—?"Ï*ãò-#?löNê¿Î2?ArKÇ;g?n³ÊJ›P?s¦5þ ?ìuª}dÜ?Á•	ÿCœö?‡PŠ.k•?"
]üVT?¹hšÕ·ž?ÀñxŒ"L?훜J˜œ?Ÿ7$ꈇ?›³÷CR?Œ…\–ˆv?¨ÃaZÔ°Ï?•ðk':"?ìK¬#ÜQÌ?° {Ž³S?{iô¤Â
"?&K-'Ö¤?»ëÿ–ÑPÀ?¯Ï~u¨u3FGL J1949.4-6140@tò$ p¸ÐÀ>yn Ç‹DÀ:Vû…Fü>À;º%—i=±¿íÕµ‹"h@Œª^¸È@vý §•[¿í5}€¼Ür¿áÄ´ø@'¿×4#H.˜¿êç…-YˆAGNbcu?ïêJU©¾?aL數©?ZîfÑ"Ò?Yø 
@ø ?P}ýíÛd?Ooñ•
?ﶒÐþÁ?~~³öŠÝ?Sœæ›'}?Z:ê§È¹?Ïd¶ÙÕ~?{UŽµ½ú0?î,ÁQüÄ?›ü­*¶?ŸYÁ~ú¡?"øˆÛd?›Fál®?$À
ˆxs?Z…â?	Ü4P­? µX2–9>?(#ÿ©d¤?‹.§?€ízvEN33FGL J1951.6+2926@Pjå?õ¹U?õh?."À9R"狔ôÀ:é'üft?ö*åS×B@T+ê¿|?ôg ÈÍcÌ¿ßs©$Ññz¿Þ'0",J¿èrNÁÙÿ¿ï9ºHfOTHERspp?t–ZèE?w5Ÿ¸Æ°5?àÙ幍±?ѳðáÉ¥ª?ßmóã$Èþ?ÑÃwH'?·WxI×ÓÖ?Âԛ&ÕÛº?Ø0ì?Ò¢?Í°Ès\÷¬?áø€¥5?Ï,w̧‰u?¿K¾Ç'?¥íØ-	ÜÛ?äÁ­œŒ ð?³QBX"?Íj£®iè½?°…™q)Mh?ÅȐÉòZØ?¹tH¿˜š?Þ$7«ïËC?ÄÎ
~Àú?Ö÷ïO?Ä	*{̊3FGL J1952.9+3253@Q2	ÀÂl@šñ`*CÀ6œÔÞF.À:›™[†8"@¯A"4Ø@'©«µz÷@Ná¾\¿Õ²Àe¡'¿á(ò"OhÒ¿æ{"噑¿ìèj"U¾PSRPSR?#arjä? ‹‡O3£A?ïõö*«ôˆ?\ŸîŸZ¡w?Q±~yÉ«F?[òŸûg[Š?-q¥Øg<·?ST0Þ$5?í²ì›†(\?¯×Õg5?²YâPâ‰z?¯È?¥.?bŒ€ô'?~²±¯/c7?íùvMÊ;:?˜ éÿoG?¬|I"=¼?•.©áÖ7£?3Øe6Êû*?4ÔÕç»??ÁŒd?…î'z•À+?‰³sIQ?…"ñKW:\3FGL J1954.2+2836@PO­K6?؀ǿáp¸À6ó®«y•îÀ:QÏng¼¨@æa³Ï$ì@ÎC°.@»ò¯Šq³¿×$Á®"0,¿àËÁcj¼¿å xðÏþ¿ì…i/ˆG¦PSRPSR?3îf ¤?9-k¸,©Û?ï‡)êí?ŒÎ='-?¥¦(Ô?u?Œ¥>Œ"rJ?@>å'ל?r[ênTP?ëå®ym?¸"t­¦$?À[ŽØC0?¸¨yd1"?v—\ã ×?m(œ¡¡=ý?ìÔ}ÊmÆv?£6À[ó®?·ûˆ6ÚC?¢›©ìû¶?\>x°å|.?WÙTï¿ÃM?íb¶ßÆÏ?¡¼u¹ëœ?´yO$þ3‡?¡eŠùðìz3FGL J1954.8-1122@=¯@Î&iÀ3(¿ó vÀ8d£zÃë}À;Oß;dZ?ó"ýèù~1@eSvŸ™Ž@+"ÿѱä¿ã=/!î¿âÝ@Š´¤b¿æ»j¥Bø¬¿çä¢WNAGNfsrq?ï±é !³?€ÐŠµ?mZÌ©-Ä?m0E`Å5¾?x]Éò"?|N¿›t‰?ï˜sªb—?‰+¿î?¶?dy:]ÚZ?i¡éW1Ï­?"ÄÆÐ3£i?…‰Ç‹ik	?íæ¼ÿþ¯b?š=TRÉ8?ûù9C?¥I÷¬0?¢–¨ð˜m=?ÄSçvŽ?î
p'Û2?›þ'ºÙk¯?q7¡8Y¸?qW÷!i¸K?¥vC«A¦?›wUÑ
Æ3FGL J1954.9-5640@uOº¿¹¾ÓÀ>üfß2*À9ø&yçL«À;¬&è¢i?ëáß͟Iv@Iè"Ïf?þ
•µ¢º¿ê³À;ÄÒ-¿æÙ~*ʦN¿Æ²˜£-Ž¿Ð¾cÓd©AGNbcu?ïÁC"Àa}?ŠÏv¢?<%*Ë¥ƒ?@r¬;‰¦?}›êóvÀ?€¯—'Ï$?ïkUAí«?"к ‡³?e<£õ?q™@í­[?Û†‡zº?'²ÜâØ?íðÈÅXˆî?uzôVL¡?—aæPHcp?‹	úÀÀ?¥B€'S?r?"xCGç5ë?îì€îx? ›jñó·Ï?aA§a‰~;?q£†"	?­]zÿp? %[Ζ&%3FGL J1955.0-1605@9 1ôoÀ5"
`:Ó;À9qá/Z`ŸÀ;^ꉯA¿à\L'ª@†Õûõ"Q@`=;"¿ßÍã}"S¯¿è2:àÚ(‰¿Ïñ¢Ål¿áû¶¡+"1AGNbcu?ïF.VÍl?›®¼ýÝ(?dëöÎ?l±påÁ˜?"œÓÃ8˜?š7á"ÏR?îö
|âQ?©b*x¸­ª?}òI~s;?ŽzѲ"?™Â,0¿˜Þ?¤½ñ÷4ÊÂ?ìåЎvŒ?¡j^¨ß?›P+³þ4?‹a~HN?²pŸL
?œÙç^¦`1?ê²I± _Š?³±'-ü?['Œÿâ^?[½Ï¸n"[?Åž6d'
?³#9œç^3FGL J1955.1+1357@J^à€øÀ;– oÀ8áú"pmPÀ;6¬¯öÓ1?ï³–&@,ëp{é@é@kU¿ßÿ¦"÷@¿æE9BkàN¿á
ЬÅ	N¿éÓÇùåpAGNfsrq?ï·ì&äß)?~ø§J;+ï?Yb蕻—Ø?X&6fû^?}±2h!…|?|;±-ïr?îÑa×¾§<?©¡—‡
à?s£â ^?€Q÷®]C? uf0 ‰?§5I`n?íá+ŽŒ ?™¦;‰¿YV?šOš†^°?Ü, ª=d?¤Åz£çö'?'Û€†j ¡?ï44"CÛ ?Ž¶ßÏÒ3<?T`ËC×CY?WNãhGJ?˜3oG'»?ú˸Ñ^3FGL J1955.9+0212@E8"åx•À*ƒõž}.)À9÷Wfï"bÀ;o³1fª¿ó*ü6i@
œs]ð¡?þÖ
€·ux?ïøjb§ó'¿ãC_T	¨±¿â.­*M¹û¿Ó`óí»
AGNbcu?ïVi"üy«?"'Cv*?PF~ض'u?P'¡÷q?".s²åb]?"Î
-ÅV?ï¹^#7:à?… òi(l?Vß%K«Š?^æ`=0Ý?}Ͷ›¥v?ƒ8Ô\͍?íßþs)S‰?–¹oæm@?• œ47?ƒÞ#M€"?§0
j¡-h?'"¬µ‹Î•?îp25G)«?ŸÓíIøR6?/ßþ&¨)Ü?6=}ûÆ?¨Üü­f½/?ŸÇôZÝ#ß3FGL J1957.0-3234@ "´ ©ÓÀ;4À_×,À9Åþ¦c¬xÀ;€­-¿ãAði\@s³û¼?@§Å_ÆB¿às¬ûԪſïþՇuC"?ï¯d3[L¿ä_Ë~GŒAGNfsrq?ù?ŽS¢jä?V6ß#Ì?b'HÊ8à?ŒËŸ{CÝ5?Œü¥Ôeȯ?ï‹&Ó|OÌ?œW_rѬ­?dÂç<š?w`âMäQ?ˆ6
02=½?—'2³Ã}Ð?ìqGHãV?¢ÕWd€¶»?šåt9$&?Šç4ð½?µ¼hªœN	?Ÿ²tt—x?íRÄ-?¼zÃå/¯?"@ ·™?Ir@
4	?³~Uƒ¯R?¼{éà'x3FGL J1957.7+5034@U&¸`.>@&G^cb¦À8(ÂÂ#&À;täǕUg@ÿ¾Šêª-@ò/@µQÜ@—çZl³¿ÝŒr'¿–¿äÒBR5¿í;u-meM¿ïÿK<igÎPSRPSR?š'=4³?­~'ÌHœ?îÿ[—–.?¯ú~F›?xm@ !?	'PwÿE?QD
['¼œ?gŠ@§)ßü?î㼉-'?¦ƒÙþ+Û7?¡D䐙ã?¦P}­Cå?Æu1î×Ó?¯Y½ù_ŸR?æ©aÓ}M?³¦w—íÉu?½Ê³7çÀ?¤$[d
èÕ?TaØÓÞ,=?TrLYËä?︻ §á?"L§ØÊóB?~‰¹w"Ì?ƒAà,qL3FGL J1958.0-3847?ø¿ÜÿŸÝÖÀ<úéŸkj²À8ƒêìÀ;GX&1Âñ?ö/R֑œ @ß*òœë@I1c$g"¿âͺPy¸¿å'¾7³ ¿çe"·'Üo¿ëxû¿S'yAGNfsrq?ïÅ8gû?tÛbß,.?pWp!-M¿?p°pÇå?jUª_›?d¥ýž|	à?ïµ+Uì+O?€Æ\ѹ¡ë?Tó¼ã¹­?]…û›+?€²è'u?}¢¦>¼é?íjé‹´ò?¡[Z˳?©×o-Ì?šËv.î·?žóÿRðc»?|§91=?ï§ÐH*U?ˆ×ç…,ï?EìÓ>#Ò?Oñë	²i3?"Ü>º-?ˆiÄév¼3FGL J1958.2-3011@%åéÞU‹MÀ:Ǎà'ódÀ9×Ç.'Z¸À;h†`Ô¿©ñ/H;.ß@œ€9¡6q?ý²³?ê•œSÞ$¿æäWôÄɯ¿Â·è"cQ‰¿Ö|âž43AGNbll?ïùÍÅÚ?Fý§á`?°tœ#̒?n•´®£Â?JqÄc&Yu?E·Up}q5?ïÍ®N«?{5U­†g2?RüJœQÆ?U^̋xÛ?yóº1•{?x{ÒÝ$?ïG5d÷
?ƒ¼Õ!R?y'‰£;§s?p:Zdøâ?ÏpøN´Å?€'ô†Þy(?îê}+öà?"7λ¢ ?Jyœœp?)
DSh?¡IˆÉ®?"-xǞ}3FGL J1958.6+2845@PxèӔ¿Öƒ×`#¬-À7	.Cà)¡À:o9ä'\@æZSÒ@'€ÊjÇÊ?ÿWS–€	¦?<gºNoû¿à`ïë¿ç¨óºÞsú¿ë¬êŸ·çPSRPSR?R£J˜9ú!?^ëÐÌ i?ï¢Ø4Xþ?'p¼?"õ"ßâh?þ#Z
ï·?v$ÉòzÓ?@hK›i'?ëiu,?_h?½V~1&á?ÂW¼ŠiD?½X™BHB?‡ž»x—{¥?†8Š¢é ?ê'þc³z³?°D‰fAX&?Äz¹¨x?®«I+4¬?L‡ûHtP?I^q÷Žµú?îl'+cê?ŸÅ'erž?¨Í_)Ô=¶?ŸlÌÞh‹3FGL J1959.1-4245@vQð€0<À=üÀu¦uÀ8šw§×IþÀ;~×¢äß?ð5b]]?@Æ&ö¶@Å»à~í¿áíÐGMû¿çB5×Ó;&¿æ`,,¦®¿ïn1–¥ôFAGNfsrq?ïàZÅ¢—?cëPå6 ?T5섹¼ ?RF²»µe?eŠîøŠu?`½{1z?ï´3ÍÓ	?€c7| ?W3¶	7Ù?cX*͒Y?€Æ	Šî?{Ê(¨~'?î_O¬
?"×ÁÓÕ?›¥é"™_'?ŠÏtž²úÑ?˜vìçå¿?ˆS"1×ïG?ïµÄmkä)?…C¹Ðo?H*ƒ\¹ ?Uƒíß¾§x?<o;em?"¦æ#>ƒ3FGL J1959.5+2047@M—ç@™ÅÀÅ)ÀBеÀ8¾í:*ž9À;2šY²ù½@)ï¶Ü @>2«#æ?ÿbxò)(¿Ò¼·µ}>´¿áæO̊Ìf¿é͉Ñ`Á¿ïÿÕOþ"PSRPSR?iS®³Ià?mJÁ62"…?îªKJu¾ù?¨"˙Ϊ?£Âv¸Ûä?§§ûÏZ^'?;ºæ
B'¨?MŒÕã¢?ìu"HI¶?·yÊ)ë4+?¼7¢Ùo½?·tÝçG?¨'
Fœ%?šSt?5?êÎÅÚ$>ô?¨"Äâ—áŒ?½@Ì|ºJ?£ìujýÏ5?ò	"—{¹?u ªzóv7?î	ÊÃ@1?¡bg|tp?ªòñ&?ž¸f‹;ãg3FGL J1959.8-4725@uüÒ}ÔAÀ>Û'ÿùJÀ99ôêù¾À;D$¶˜­á?õÚÛö¶U<@9Üùë"â?è1k©,šÏ¿‡Ç·—¹ù¿½	[]ô§Ý¿Óâž/Ö\n¿àSݦ6AGNbcu?ìO'¼ÝÉ?¼Îù?©M0–戚?±2­6ª •?°ÝQӕÍk?·'̖8?ì›eŠ=ù?Â~]UÖóœ?¨íàáW?¶:±ùó‰/?³"4ʽ"‹?´NcWø?ã8ò±W¦ø?¸18©÷ìã?Ϗ£ÛXv?¶S­Î_?̒ƨ?­"Z`ϘÕ?æE‰Þš\?Á=†ÂÅcÊ?«…L#¤:­?¨áH'Ì×f?ÐEgÎCô?Àúkb ¦»3FGL J2000.0+6509@X€Ì¿Ì3J@1ª_ÏspÀ7h¢q¯oÅÀ:¸aÏþ°u?¤âÛÊƬ@B"FY?þ!±á9u¿Ù¿Ìhù¾¿à2'U†ß¿Ú´Oñb‹ï¿Öƒ×¢¶PAGNbll?ïïg¹ª	ã?dĶþZW?0õ-WŒZ7?7¨px1—?\óAV	 [?c''eœ?ï¿Úo*[ù?‡ÉEb¢ò?cu»Ýü«?gÍYêçÖx?vWêäã=?…2/".Ü?îm%:3z?žrwëä(Ò?€gËs:1 ?€ÜDÑÞU?£:ώ;ó?›Yü$Oz?î×`¢;Œÿ?"nñX¸)­?.^ƒ­'ç7?4ÏæeÝ?¢k—X™­
?"Vi_co~3FGL J2000.1+4212@SaqýÌI@ªE`zîÀ9A›\è8cÀ;!ÛjõA`¿òöƒ—¤¡à@ÅWìÐù,@¾3Ÿi½3¿ÞšXFú ©¿ã¨ž÷k÷¿êŠ"ë"çû¿Üö§‰‹AGNbcu?ï§Ö"ì?¦¨DjE‹?m;–‹äÌ?l{Ÿþ2b?}vêDw ?}':póä!?îÁy<y4?¨"«Í'˜¨?goÑm­?r˜ûŸª?¢vµB¸%ù?§·9ß°˜?ídAÖ¦ÄA?žm¾ŠƒØi?™zþãOý«?‹¤qü,§)?¬þc#ë½'?˜æÙuše$?îÛ0æ'…$?"¿\ϱ?7Ðx@§0!?DȜvÙÍh?¢P­_^?"{"†_Ž3FGL J2000.4-2926@'Íä ¦hµÀ:ÿyŸÿhÀ9WMî \+À;jE­‰:§¿Õêú†÷ß@c²åE°@ÕúÁ;t¿é†pÞÓÇ¿æÞSèO¾¿ç«v-ƒÆÉ¿Ë1Æñ~YAGNfsrq?îùNn#QÏ?º(Šã7¯?tÙBãûì?9ùÈQŗ?›Ð»êÜÇ3?¸b;š…Ï?ïȧ'U?¸H?<­¶?eb§è{?ü?yEsÑgÆ?†¡£ÛüšÃ?Š%:W?ìüÉחŠá? "Ëþߧã?Ÿ¨!c+è?‰
•p¢!O?°±Ç:êÞ?™c?m?îÈADâ? °ÆWéÈk?R"‡»yøl?[`'ùj /?®îרOâ? ¬ƒ¤C¶A3FGL J2001.0-1750@7ýJ€àÀ7%A` JÀ8…Þs¾=¾À;G¯e³¹¿ÙLAþcXü@¤Ð.@z+µ—Ò¿â@0œªñ¿èö‡Éëúm¿Úê"65ú–¿å"ì0•IAGNfsrq?ïö{ÐÚÂó?U"é)ÀC?
¶q])Ã?Ø'>
?R (–ï-?TÉÄõÁ•¶?ïÆå{ðt?y°¬Zv~?Q!Œ$ª?W´Ô¸‡?x¬"Þþœ?vÁ´xk7?îöIÐoX?¾ß Ô¦ó?zRÇ#¼²:?m_ª©§š?š¢+=è"?‹iJHHF?ïÊ2Yº©2?s³{ê¿«>õôVIju?q~ðÆ<þ?zÐß"U?s«c^÷ir3FGL J2001.1+4352@SÄŸê³@s•À8–À7Ô¿ª¥À:k$;H«?ÓH îÀ›@T/(6ªâ?ÿŠsž³3ô¿àù ÀTnl¿à8îCȊ¿Û:K•Õ"Ç¿ßÕü#°AGNbll?ïZçF¤?˜Y)Â>z?C®VJm3·?F_ßdH ü?"©‹ƒÁÝ?˜*"ngá?ï<à)F²ì?ŸÀ°ï(s?^p[à?g& `eËn?–'sÑx±ˆ?žNhEØ9?ë'¬¬mò?¬é·Ø·?'u¦L/§?‹Šè†åû@?¿Ž¢±	"Œ?ª"_>{?ïm•·ä'ð?Ž•¥èsn™?6ìOg?*Ėj9…?'=½g÷šs?ŽIýé'3FGL J2001.8+7041@YÕÑ_ÄÖ@3õÕߛªÀ9‰´	‡h?À;""²Çì?à̈́ò\@
‹oK<ih@§`¥aÏ?ïŲFŽ¯±¿ä—¿iÉ¿Õˆ&xqi¿â:&ù$TÚAGNbll?ïcÌQØ×?"^§ñ·"_?yÚEGBÆá?yfµJ§*ê?ŠÈæ(փ?'Æ»^dþ»?í\z#¡‹A?º•¹uÕéc?¦IP›Ë?±Y3Ü	æO?£ïE¯–°?°1ɨô€Ú?í˜ߨé?ž"#ò/õî?™‹²:²:?‰àL×ý?©ºèQ?—ç${Gìn?脎þÝfk?º"grrÆ5?ª0YÑó?¤ŒZZŸP?ÇløsñÕ?¸: œÃ?å3FGL J2002.7+6303@X
FŸ÷¬@0oò ClfÀ:i¨+,ÔtÀ;á|lb(ê?㙵·÷'@ý&±ÅŠ@#¿¢Â¸¿ä¡?[pz¿ìÒu³?ÀÔjÁÑv¿ÚsÜ
­XAGNbcu?ïÅ0pîÛD?ŽlÙµQ ?8rýuê9Ü?9Ô´WÕ3?{à—±3ºÇ?ŽK×Ë@'?ïW4Ý$<?¡U¬d
Î
?uFL?%\?{†-Ç´"é?ñ¢—^µ?Ÿ®l™ƒl?îØ
œ?Ðú?Ž!˦ !¬?'ÙŸ[Ui¸?r5I|WÎé?›'|Ê[+Ë?ŠåiìÎ?ï(
Lû-?"ýLø°3ð?Qú2Ü
Y?h*-"xæ?™ß2Ú¹?" M,š:3FGL J2004.8+7003@Y¶Â!y@3téÅ+À9ò	7´À;‹ ¬Gò?°Ð®q¬x@ÏÇÓé¢?þ©€Â]2¿å÷\UÉé¡¿â§ÆZÂÄ5¿Ü¼»ŽrÊ¿ÇâzwÚAGNbll?ïõövØ?^ïdJ‰x?)jòˆüö©?'dN)@?R–Áò±ò?]昔ñ½?ïÉó!7"
?|\'é%5?dŽÍ?g¤±µbå?p¾àwB?t¾J‰5O?ï–÷4{Ä?|#d‹ð¥?qu½Û6/?mÖUhâ?‡T
†+?uù&®Šë?ï¡¢u?|(؃¸­á?'鲑Þ!ý?2q8ø.t?‡7»õ5¼?{õ°Í'?3FGL J2005.2+7752@['¡ Ï@6¿¤Ÿ‡dÀ8š°hÀ;~¹Ù«?ôÍJtm@Ët‡ff;@¿Ý¿ŽJÜ¿àã?˘¿ãÄÊPà\¿á©ðìçŸa¿ç¥eµ2ÒAGNbll?ïâjù-\é?hö7˾£W?[H3ò^©T?["†
FÔ®?_áٲ熼?`=|ÀN\·?ïǾnÝ,?}™mf4Ò?hSڙk?lÊ<?oîڂH;	?sÅÞ+{T?î›\q>Ç?•Ñj£"ˆ™?–¾@¶Yn'?)BÈx©?•Þ»~¸¬?‰LùäC-?ﻥ©Z?'<ã"JJ?Q[býLÚð?X)ŠYôZÅ?}ÖR´¼â?99roŽª3FGL J2006.0-2311@2ø÷àvͽÀ:-Z@¾61À9/?ÐÐgŒÀ;}|Ùor?îŽ"é+@hö'äöd@ö?ŒÝÉ¿áØp+â¿çrDoè脿ë™IÙõL¿æúÓÓ§1ˆAGNfsrq?ïö2ˆD?PÃþV	Ì?B…B°åïW?Eª-ré¸?Eôàùd?Gq›D5çó?ï©1fÚ?†/œuî‡?\+]«qG?`X‡¨Õň?'=6Çðۓ?"zª<âY?:µ™A?i]=M'5?‹«¨Bóî/?}xÙ7:?œ¶ä‡ÒàÌ?‹(S1½"?ï,-½€™?"v©
œ?h»!추?møí'Lµ?—bä;rV(?"ËOµ.¢3FGL J2007.3+6605@XÏè?ïÚ@1n´_î}!À9€ú:þÀ;'-±2ã?ÚQð"
yÌ@VÆwÉS@·ò ¿ãn×Ѹ™å¿ê°Ïb «¿å0Ì6àøå¿ïþ•2ñ]ÀAGNfsrq?ïëeH×ÒF?hþÅ{ä8?;_dՊæ?8)ØþE?a.Ôۓ	x?f»,L»ð?îÉo—Ac? B
FWí?Ë¥ûŸA?Šå\¡Ö?–g4D?šc÷´•?ï%ñàæ¾|?ˆ½B/fê¤?Š^Üüu=?~<å0›£?Œu(éSë¥?	`¿Ém'?ìÞD"P1?£gÂ@TÓ!?èn–z(®?ûÀ"Ѓ»?±"ÃEvôL? ø÷ïíh3FGL J2007.7-7728@sË/ŸËÀ>Œ6`]'À9sÔöfú
À;›wï$æi¿°áõ"x'@ÿÀ+©§@výòÿf¿èz'V?ñ¿äòu¥Õ¿é¥þÓôÎ
¿ïÿ?9!AGNbcu?ïö¶Q2·Z?PN 'Ëúò?Aw!‹-Êî?@ƒ‹ñô@¶?C¯™©ôϔ?G&|¢ Ÿ?ï‰aí±ó(?†1ʒ6{?c]çð'ˆ?f{e®Ý?ˆâí‡É?ƒíÁ¦lø?îÎ8üG¢¨?ŽémZ™S^?•;mrú™g?†ê"P›Mt?ýs¾?  î'¸?îòF4*,þ?• •'C?s\èûÒu?xø¾a'6??œßÿ;ÅßÙ?'Š…pÅz3FGL J2007.8-4429@v6Ê?‰'ËÀ?ÕŸÕó½À9ŽTEÒr(À;­†Q¾8µ?ÈE'² ¤@F´šQ@¿œÿªšž¿ã>w"k4¿æä,J
æ
¿ë:ï.˜ç¿ÙÁ6ÓÉÆAGNnlsy1?ïáä|-ÿÝ?iwïÌ]?Q»Ûhè?Qû*A"?e=–ù¿?fh÷òðŒY?ï•6Åž?Š×³g†­?`'O­¾¾?y®ô+Ž0?†µÎzÏè½?"çp•ãt?ïûYÝÃ?ˆ?B­
#»?'èÌ,ôn?v#BhR·Ç?–š~J‹?'Ð|]»w?î×ntªÊ?–Ü–Pe
?aôhë	ßì?c¦•6ÎP?¡iØzµc?–Ë`æˬð3FGL J2009.3-4849@uæ
 '§À@LZ&–mÀ7ӊë€ìúÀ:©³%[Ú¿íükl@@€¦Kٝ@?ü_ãìŸP¿Øfû"¿h¿ÛvÞX»X¿Ö2ä%Pi¿×-	þ±vZAGNBLL?ïîÓ`é֝?`ë8u9k£?ì÷Ië©?Q@µà»?`°ë9Ð<·?`©q:Žà?ïÆì£øü?x´="š?Hªÿò±»¿?P€i•¥6•?ytN€­J0?v…?ú»td?ìu˳níª?ªucø.Öª?êÖÕÇþv?‡uf`d|é?¸"G‰Ï'Ü?¨à¢âÍã?ïÂÜðú?'pY? 	O>ïÂ2ݗ¡z>ùã"IfÂ?c¬7&-Ä?'nqMëä3FGL J2010.3+7228@ZVhÍJ¡@4$WÀ±5˜À9`¬é·À;Øwûº ?ö" =͕õ@Š•DË6@£3ø€ñ¿áí¬¼ó!1¿ä+ÚûIóû¿å{ÿUò6$¿ëêHeì»AGNbll?ë[ùš+îe?º'ä¨øh?ºæÿøhC´?µcW¥n5?¤rflp'Q?£±{5‹'›?èáÁºÖʞ?¼§7Ñö ?Ä÷'šOö˜?µ2>h?®™éS{Â?®øÃWmÎÎ?å´ý;¯V2?µ7¼éq´?ζðÇÏ'?²®ê‹Sc?´ê4'ç*"? ¾+¹½1?å	9¥…?³	­¡
?͓rTÜS?°_ËúHÕ"?¼³6?¯v¢š†‡¿3FGL J2012.0+4629@T"GŸÑÁÿ@ƒ32ÚÀ8PݝÕh}À;<äŒÜóÀ¿Ï+šã@Œ=AT@@Ü= ŸrL¿ä©‰[¿ã÷Z4,¿Ö?H=9$¿ã0I'f2uAGNbll?ïѾhm4?yK:N¡S? »ã¨j¹?"Þ£4N?v Uج"õ?xòkÐ/½Ê?î`Bb- ?¹ºž†]ˆ«?büäñ'?nZT['¢?¨ÌŽ?¹bM3na?ír{û@2ú?¢ôC©s?Œt A"ã?ƒ³öêØ?°ÝœAöCÚ? W&&+@¯?$ßNì?V¡=w¦Q>ñƒ'Á4?i%]þØ?ŽÕuìd?Q^3FGL J2012.1-1643@:=ÓÀíÀ9)?O¡(À9´a¼æÀ;°}À?`?û+çpÌ@¦5þ¿Ž @æsžg}¿Ò&ÞJ<}ù¿ì—ÁÜȇ2¿ïôƘw§ú¿Ùú39Š²˜AGNbll?ï¬B¶ä?Ž•Ò)'4?w
³nùE?'Vh҄ëØ?rÓñRe"?€™®i?î"öá×®&?±Àâ:é~?‰X‰¾ú?›°øòj? L»À=íö?©›%äé±?åiPÞ«´?µ$i¡dk ?NJí»G÷?¯¢{ûäÈ?Âo¼ÎÊ	9?­!®t'X?êÄÁ?–Â?¾CJâjÉ¥?³®cÑ3	ç?º…3žþ|Ë?¶+'6X@	?³b§i,,"3FGL J2014.3-0047@Dýžà*w£À2ºÜ fèÀ9wU4åºÚÀ;Fù	q?Ø&‰åz `@5dЏ$ ?ýP!?Àµ?ç]G¦²±Ä¿áÙÅ(yØ¿Óè}†­G¿â'²Íƒg9AGNbll?ï÷ØUŠ?JXLž«?!aÄÕÀ½G?¹þ…$´À?LG5tg²?I4ÄåGí?ïœyk14ó?Œd""
O@?a\ëª9a?c9წÂ?" øÈ4þ?‰¹_"3?ï&¿µ£#?†5åµ%´û?'=YBX?uÍÞJ	-Ï?'	šÜ¾ze?€íèæƍ§?í"ÔdŠŠ¢? òˆ-,ž?XŸYª?WGðAW0?²ÿV_¦F? ËŠK)µ3FGL J2014.4+3606@Rw	ÎÒa?éƒ9õÐôÀ8íaö•À:i"ïQ0?õ'2T»ï@xq5¢NI@0~ÀzY
¿à	Ç^ÎÂp¿ã­¬`›¡1¿ë>H:+tù¿é&¯â[TeOTHERspp?njí	1Ë«?t¿Dý†x£?ázu]§Y?Ðý6åÎS?ÜÄ5;2M·?ÐýôA•ÚÖ?›ETª£Dª?µ(Uä'Ì+?Ýàü="´?Íaöy²›ã?à5W;á?ÎÌ2°nN°?ÁNG/MÊ?¨—+àFwï?Õ™5ìhS?±h^D³?á¡™&xe?³…Föÿ?£Â*S°&?Ÿ³³
Ÿr?à"ªy¸ ?ÆtñO®qe?Ý`€e¹?ŀ°ñ6Óü3FGL J2014.5+0648@Hw V·À.€LÁzÀ9o>À;T' ¦Ô¿Ú}ôÌ_‰@fSvt¦p?þ¤®àþˆ?çW­ËÕ¬¿èU‰%û^¨¿ÓïKº
ß¿ÙvŠq™±~AGNbcu?`"æ2?ŽÔt+«ÛM?@ÝMN$f?<»vHt-‹?Œ"ê"q'6?ŽŽÁU¡ú?ï¥Së§ùc?˜õ¶cMMæ?]ƨµnºÖ?a—ÄÀ{U<?'ò/ÿSÏó?˜"
'¸}Ø?î³­ÌÈm?˜â[¤4å?ªŽé;Å?~¦É¢·º?§O}®¯[O?"`Ê:6âž?í.¦¤»î?£9IÁHÐ?Aº~ƒVbY?F9ì\ÂÈû?¶gUâ+sÌ?£)ê YK@3FGL J2014.9+1623@L®¡@W%À$;ÿwDÀ9Õ(X䝤À;qhµËÿG?ºâÌÆö&Á@%2?@G]Ÿmn¿å‡'(Ap@¿æQ(óØï	¿äýt½1­¿Õ¬s¦jãNAGNbcu?ïÚäŠó? ;zŸQã¯?kV§IBV¥?oºÀ³È4%?šΕÆV·?Ÿ‡)d)°è?îqŽÌÆ?°`ÅNrß?zÃT²ãöÎ?'ÏsY!¢Q?ªý¾P¶´É?­D6õ¯òM?îI—١ܐ?•¶®œÇM2?žTœ²ß×?~Õ*êÍÄ:?£XˆÇ?'Jú¾w(
?îµ@7Žj?"%6- •?UQ	{0øË?YÈËìnnÅ?¤v°­'Ÿ?'ÔÚ<ê÷3FGL J2015.2-0138@D§:¶~­À3XhÌÀ9%¹˜<¢HÀ;^||R`ö?ì8_Œ¤àí@
Í,݃©B@7* ís?±F(mÝS-¿åð"Ò.­à¿ã‹ü]¼§C¿åRÜN[>AGNbll?à+åE™ç?ȗNÊzw;?ÁY("µ‹?¹¦è
ê?Öû¡+›qk?Ç
c*mTR?æb™y Ô?ʲÂ,mF?ÄÁQ%Õs/?§l'­<ô?Á¶€tD	€?½qB÷^×Í?è]¢'7?¯ü˜²~+?ºïOÁ³<Ê?£°œ‡Ë/Ý?Á%•Â?¥#uëòl?ܱÝ—­ž?¶[8ìÆ.?ÆÅñaé¼?µÎ"_®Â?×ì_é·]'?¸ãù©9)á3FGL J2015.6+3709@R·_ßÏ?òø
€CRÀ7Ïng¼¨À:+l¤nò?ÿµðÓ×@rõJð>@@îݘͿáÞ³&¿åÂóýé$q¿çxýP/¿è¤ï‰ÌXDAGNFSRQ?áx%÷[Ðj?Ìçkä%[?—2ï@ݐ¨?—ôã?$>?ۜ…:†!?Íù±§˜?⎞ƒyÈ?Ճâ†Ð>?Ž±"ÿ ?˜ù
ð?Ùí9ðXÜt?Ôû¹%>›I?ãx‰W 	¤?µ'ÖÊ?¹æ5áÕv?¦S€*À
â?ҕ`
Çw[?´9ÁÖ/®?ìÏÚº0?µ¢À'îD?x6üŒXX¼?‹˜Åȕ`Û?¾^afpø?´Ï1¢É*3FGL J2016.4-0905@A+©Ÿ¡—À6úã Ì(bÀ8ࢻž§À;Bqÿ÷œ"¿Û}ˆ¯šœ@šÍ¥å­C?ÿÀìÿÈ!¿Ý(§¶_D¿ßÙ.ÁÌk¿àFbuž›?¿Ûj?ZD*cAGNbll?ï÷×Âƛ?LFŠ''2ë?$ÕCpµq³?(†7!{œ?Kn8¸A
?H«Š3À§Á?ﺊo=È?€XT*èC?U5F5QøÖ?Yº[_«?}§é;û?~ZCâÛϹ?î߉½¢?9Í}¢K?…üK®È[`?v÷[íœ,?™¢…'¹?ˆl¾"Ó1?îò/ŸÕ›G? 2|H¾?2š²–?4Ju 6x? ·Ðz3Œ?{.+[¡Â3FGL J2017.3+0602@HOt cLÖÀ0:?–îÄÀ8"úgðÀ;×@Än@ƒ–ÿ‹eú@
S
ã2ê¹?ö'ª%Øם¿Æ‰Wu:rJ¿Ê£ö¿º¿Ü÷ßFïJ¿ìÁÄÜq
<PSRPSR?=ç=Ò}?A%¯¤‰_É?ï~'£ý@?êšÈcW?r×ÆÌ?²»1÷';?]l›–»?zEô›ÃÇù?î¿[KÆ?¥ Ýèq¾¯?£#:*¾"š?¤çœÅ­C?¨‡7Þ|ð?ÃÂSܑ?뗖°3?¨˜~¾¢Ý¶?·5&—ð?£ýÿY''Š?sóXàis|?oÁºÈsSÎ?îpx(öŒ? Y¯ð-ä&?¦zT'Xà?žhN`ƒ@3FGL J2017.6-4110@vz4¿ÍhÀ@À?öÀ:få2õÒÀ;ÉdÞב¿å	 Å>ÛT@
Lº–@FônJ6¿ÛýxU¿ìæRµöп´U¶ÀÆÚ¿Ïš¼ÀvAGNbcu?ï´MåšÄ°?‡'пI?!îrªÜp?"Ma줦?'¨'ß"(½?‡vê–,ãž?ïÅw՚}?wÙ#ÎϹ™?K¸[•b¾?RŽªç­¸?yÍŒö?vÀÍaªI?îg»‰âÖ?'¡fÇ«_r?‡äK´?uI¡US$?£•Ñ†à'i?s/HT1Ü?ï{m©Ƀ?ƒì™¤|Å ?Ô¿ÌX?œ¥ÅWäK?‰`ÒûïÃ?ƒî̂Gïß3FGL J2017.6-1616@;F'À9@"À:7{ßto>À9J
'/ï²À;rÁ3;–¯?ðºÌ1qg @Çö‰^¸ó@ц B« ¿ÊnЖ
¦¿áÔÇq\þM¿×'r%-ÙO¿î.
)y¡PSRpsr?ÔÏß´îP?È1-<yÆ?ÝçûrO™J?ÊZð?—2$?ʐI±"°Ê?Â¥]_ˆïÞ?ÙÁˆ¬{+?ǧ<û9MØ?Ö踙ˆEo?Ç¡'·	ÖT?Ϋ}t²~Ì?ÀªGY?ÜL§Džn?¶rOþZÝ?Ù« vÓ´À?¶
"Õ@Q?Äq%ÃÏY¦?¬RF6ß?ß¾*Ò÷ûë?·‡ºUPk?ÉêìSJÓ?ºwˆþì/?Ӂ߶Þ^«?´&RvØÅ3FGL J2018.5+3851@S%öà1-Ÿ?úžÂÊ £À8­°"—©ÕÀ:'õ}Åþ?éfÛ+_T@â»Z^›A@Ô6€šš ?ï·¸ˆ¿æø…cF¿ç{g;§¿×}–³é°AGNbcu?Ðp½¯þI@?É2Цxé7?¸{l³
Ã?·Ãd¢Þ7?äÄQºjy¨?ÌÓé…À
?Å«Z-©h@?ÎZ0ÊÖKé?¬+6`·‹?³‡˜jÖÍ?èÒvŠ-@?Ï»äfp?мª76'Ò?µ}Þ±£?¿ò}Éß9M?§	¦8²gI?ã£[+)î?¸ÿ
R¾Œ"?Öma_ïìI?¿…nýML?¨‰q áj?¥ÈÌ븁?ã@¸=ùñÄ?À-þs™?Ò3FGL J2021.1+3651@RÎè_ÐJ0?¼éóŸÛŽBÀ5hÀwSôtÀ9Þè¬&d@ŒN¸@ý{|@ÛnÚ~;D¿ÕT.wÙø§¿á"~ièQ
¿æ¤7HÛTê¿íCÜq8/$PSRPSR?I§Vc"~?ÇÙ\¨Š5?ï©|à?'ÖÎ	ÿù?…®§æ´R?'Óõ¨•Š?AÞ¶›>`R?|ܽiZ&?îÆiċ^?§ÅJ4ïaf?£QóÉJPž?§«F¤QÔ#?j,7LÙ©?m@}™Ûgh?í5ê"¢Ü?¡éÚ+jT?¶Tîô†ÚR?¡Ò¬¸z|>ö—¨›¹«Æ?›±èÓå!?Q D0?‡sQ¼$æû?ˆÈßáq?‡gvP
‡3FGL J2021.5+4026@SŽÔ2Tç@ªJ_ʕæÀ4Øï;Œž	À9҇'§
ö@K§ÍäÏÎ@>=@§:@¨[—ÖK¿Ók›
På:¿â*›Ö¤¿ç­»I–¾¿î9ïxPý&PSRPSR?¤1%ônñ?³BBA,µ?í»YŠaž?¼‡PTòt? BAûg+?°ñ^3²h<?V¢R~bxÀ?||ÔSԜÉ?ìο¶×L?Äp$U	hT?¹/xÿNsÇ?Ä3ò‰Q_è?¼í-!Œý?±SVZ‰ß?à1	°'á?½Ý
Ó/©?ؼR¤;Ù@?¾Â¢ä¨º?3×+Ýò9=?=xcÛ?ïyˆAîú?¡et¨Þ?œrHJWé?¡L×"Ãrv3FGL J2021.9+0630@HÐu@ýAÀ0ÅM¿¦sÀ9ªwhiÏÀ;m
[£"Å¿û»T­~«@
5#·j:@s\ <`ƒ¿àJ"+y3¿à`™. 
¿á‰ûcZ¿èø°1ze;AGNbll?ëÐsՈQ€?¶K}hËÔÛ?–Im®ïÀ?—o>QY7
?»ê xQ¸?´š ÷}+"?b‡—õ?•Ú¦¿c4V?j>e/7õÝ?r°ìöJ°‹?ˆƒNLd?'–èNjyÃ?ëð•É­?¥.J/"u?©Wñw¤…?—'3• ë?³ÏXû·`T?œÑLçA?îGž@¡#?¦VF§°ƒ?N,…¥}Å]?_ƒ¬|â/?®Ô_öË?¦?'T"3FGL J2022.2+3840@S6¸!ï?îÍÁ¿Ü&À7û_)[CÀ:G$ãW²@Óï` ~»@
e•ÙE¬@xH-Á.^¿ÝÐdÜÎw¿è‰œ*Œñ¿ë.P«>¡¿ïÿ†ÈÜ}DOTHERspp
?d_Ðg'r?m¡Ç¦äÛ?âê_åaê?Ѿ8ß¾<ð?Ú€"n«)?Ѳø5Ê#ô?9ýÿÔáÌÇ?Vèw †ÅF?ìÿIçûEÅ?¶fÝ8FR	?·ë²ÀPð?¶g ÒuòH?®¾}5‰? {¨wìb?áß»öÒ@?¸€Yþƒl?Øh¸m"ª[?¹lö/ã'†?^Lôg,0?Y|ã¾7ƒ»?ëï,Ýr"p?±{=-¿?À
ðLãæ?±PYgŸ9y3FGL J2022.2-4515@v.F_•'ÍÀA:2 f<uÀ9°Ö?<VÀ;»>©ˆúæ?Õjˆ6<I@˜þi'@ÄAÿÿª¿áq—->㧿åõ7¿ßÔf¿æ‹"\!¿¿å³N÷^òAGNbll?ïpĕØ7¯?"mî _A?uAP
'àJ?yÂÚ酩?‰.2ƒ^#ü?"Ç.'?îã_tVoÆ?¡0ûB¤'ä?}<ËdSw?Šß-¹A,?œDÞ±Xò}?šò"ñlò?íØlMûr‹?šÝ…V²¹T?"m˜_'…?'EUbùn½?¨ÂoCm?•ô™B=ê?ìÝXç™\c?¤¨)Rü*?ŒÅXq-
?'È¥›L¼?µ|¿†÷R?£ä•bÐ^3FGL J2022.5+7612@[Sc€ß@5#ô™=SÀ8߃'gMÀ;€Å¤º_¿¸AÅ(£@Ëbôkø!@ÍÄÀcÝË¿æ|V'0¿äs ¾¦ïC¿äYž¿ʵ¿æX
6n|AGNbll?ïµúÄÿä÷?'²yX4ÿ?k<ËãCÅ?m¦8螴?wd7Žkþ?~ˆÊUBGÿ?ïCÉ5R¯þ?›ã4_nÁ-?…¢ªA0p?ˆûYNÞÇ?‰kj#F?"0œ›H°×?îÍm{ôüU?"åx-Æfl?ˆö}¶íL?'O¤ÉÜEq?™×öþØ?âyd×?í•êŒçç&?¡èm'½á"?†&ê£}Üß?'ِæò ô?°‹ÎDQ;? Ñ‡ïšm)3FGL J2023.2+3154@QÙÜßÔçNÀ']ßYAeÀ9nwºKÀÉÀ;6jö ?ëÐ^_0çÿ@ çiõ@'x z´Q?ížf5F¼[¿ ;'Z鎿ãZsæŠA¿áIÑJ¾rËAGNbcu?ï=O"tÉ?—í†ûË-?y*ÔÍ¢Ô?yI‡fÅ?' Úß²?•ºÐå¹Ù?á·A£›u?ÕÆTÂ[À?®-'ÿÓ½w?²‡lÛ<?Ø̾Qf?ÓTBàâ?ìˆ9Ђ?¥ƒr»rï?£3¿jÄû?'bƒñFÐ?µÙÞ®äx?¢-½>þ?è?jÇó?·¸#îÄ?²'Úõé0?¨Ê¢ÂyÒ?Ÿê'Éëž?³ø(²>2O3FGL J2023.6-1139@@O¢ŸÒ˜¿À9®â_ܪÀ9'`uÖFÀ;T3—Ac?ò´bÞ©ª@µL¨z2?ÿV´öí?¦,EG ¿­¿ÚZ"|<ø•¿ÙÆ»®ÊáÄ¿çz8B'ŸûAGNfsrq?îƬ—›B>? Q¸k‡¤?'΍ÆD2?–hJ[?"[ßFS†!?"žÏtÍ?í6"ò©~?¯Ÿc›Q
? âx¶%݂? "5
ðZ?«»X)oŠ¨?¤Ôh'Zl>?ënøç›?¬jkiíÀ?³'[l®7w?£@Š
bât?±ߤïÂ?ž¥3Hˆ?çš]ÄQ"?­†3—U?°ØÚ'm?¡ÔEüz®?É+…y%¹¹?«ßí±rFä3FGL J2024.4-0848@AƔÿÖåUÀ8££Àd¾À9¹Í°!›[À;[Ö¥"¢à¿Ð&m2ï|¶@—pÛà;?û=ßÿ¯x(?ìñÐÖi%¿Þßo1CD¿Ù^ß§¿È°ÂHB®AGNbcu?ï÷øº§P'?QT‰ôwA	?"@á—ÂÏm?#,¢o;)ý?KŒÜüÍ??P–ÊÓµªå?ïÅZ@èA?{HÛRªÏ»?RýD…x?UŒpŸ7¤Á?xðӎjM?xá"òL?ï>|~a>Ú?ƒÁÞ£"?û¥¥Z@ª?sYGê¦Ä?1†Ê"r?€'ñÊlÝ?ïÀUxËx?u‰¼I_¬?$Cö–¦?15¡ÄˆË?ßoBùoÙ?gdŽ'A3FGL J2024.4-3254@#>óà¿À@n¦`QyoÀ9<ÚvÙ{1À;@#¾†À°×º'‹Ù@å5O?b@OêÀ'ÍÏ¿éÄ:ê.)¿çØ
Ù¤¿âÉ	7¥ø¿ï¢3äÔAGNfsrq?ïù"êþ?QÍM~ƒ?1ªîGù6
?5Él>^2?Bñý3ûg¨?M@8Qhr?ïÀÛ§+?›?{¥m¾"ÓÌ?N§i`"?Vîø"e)?{½:]?Ƴ?xœ/²|¢?Á.¦ô?'ïO>ûë?""bcdJã?…ÕÉÐ;Y´?—Ü%vÆ֎?ŠUþ¢N?J89?†÷'M!<á?BÒ«±™?+ŸWëv]?€ßҟF>?†âpÝ׈ô3FGL J2025.2+3340@RF–àU­ÀOÖOÀ7é£?4É5À:^zb?øÐ{ùF@…'Ԇª@ئ²†Ði¿â±Àç]¿¿éŠù‡"³¿æ"@¢Ã ¿íÍVœ2¿àAGNbcu?è¨néI€?Äà2È,͔?±¡f]¥¿?²h!m*ä?Æö', ?»»%¬2?æÓÌÙÀµL?Ò0k4¤Ýà?¥£¼
f׎?´Å&N@j?ÏGݖctí?ÐWu´fÛÒ?âÞÜÃã'?³õÜ©¿ùY?ÿíÎ;ƒ?¬wâ(ó"?ÐcÏ_p›?±0\;Aªß?ê Z+5?ºv¡¶ÞÔ?…è?–Á¨?½ž¡à%è?Æ Z[?¹7¶£ï¦3FGL J2025.6-0736@Br® 9[kÀ8d:ঞeÀ7Wm¯0ÔÀ:æX"»@ܺ«@7ï<ä7@xãPÇÄ¿ßRáù§u¿å¥¨×¶F	¿æä¦É¿ëÁuuoe5AGNfsrq?ï0⣹?ŠØ;œx«É?{ÇP
j—N?ƒ"P|µŠ?ÜKÂ!ÆD?'°)+ᗛ?ïÀ‹d'=?}îË®ãv?VØbvA¼?`ÍÑh¸?z:µ!Q??y™ɸ=?éenå®®?°"²ç§9"?¾"'™Žˆˆ?§Ý)o›¦™?¶±÷=¬?¥yzrZ?ïäËS ³?uJºÔ¦?!²‰'!þ®?TpÂØ°ý½?jƒÆÂ,Ã?t'3Çõ	3FGL J2026.3+7644@[z°<«'@54·¿õMõÀ:"TÊÀ;ÐóöÝA¿ò²cЦ÷@·…:<ý?ým8ÎAl?ì™Nw©§%¿½†"¯¿ÜÞj)К¿éäÁªÒ'AGNbcu?ï0c³°Í?œ»k0Ö§?"£Îªú"?˜S2ˆŸ¿?y>îíŒ@?‡'€ìd¢?î\ãÿ»P?µˆÂâÒl6?–ô';æ¾?ª˜Ž7¹?nî̯A
?®.hO˜?ë~ñYnÊ?­¯9V»õä?·ä»m&«Ú?©_­(ªª^?¨GsŽÒKŸ?•\ï¢iª?íÜT"¥?¨øHù»Ñ?%, Ë®?›ç÷g»Ï?ª:+ÈMoà?£|îh÷`3FGL J2028.3+3332@RW€dÀ	¾ÀD©'À7xrϏÀ:pŠ)º
­@VVù¶æ@}$îÌÑÕ?ü£_9M¿²²U/åÔc¿Ú³íéä¿çýuûÉ~¿î:öå¥PSRPSR?0¼®¬]?1ª›‹™ò×?ïŸû™ì!V?‹@3uR?‡{4–±Þ?‹sAã¬ê?¬‡[¬D?=­
Að?íE%X¨ÀÝ?²`yÁëº?µÏj5˜"/?²]OÚØP'?vñ›¼2Ô?r
-n•?ì¬Å¢[Íâ?¢^sÿÌ̃?¹0óÓeÍÈ?¢–i'?^éâ1Kµ?WŸN"ښ?íÙÕç/ƒa?œDW'à÷?°µ©<GÅ?›gß«~·3FGL J2029.4+4923@U˜WŸúë@Z
@JÈÑÀ8rÞN«_À:úō=jÅ?óÁz´&8@o*s*©@I:ÀETô¿â½'ö{-.¿àb|>Œ¿égóI8X6¿ì
GÃ^vAGNbll?ëÅyº8¨>?·ef{Û¿?º2¢nîŠß?µË¹Z—;Þ?ž†>ý0ÌÒ?žß'ö7?íS¼i§³{?¶}:"×°?'`]‡3†y?…·V×1"?³Ûó\?µf܆ǟ?æŸ`Òɸ?°"+~Ž(?ÅÔÐæý1?ªÚèÔtÁ?¿[]coP?§€Ìi1H?ì6'¡_;?§äHqg¼?¡ý¾ve‹?»nC	8Â?µL¤¡Óh?¤Ó¤g3Ì3FGL J2030.0+3642@S~ +ïr¿öçÇ¿Ç«¦À7΋ýϤÀ:ž;aÕÝî@øByw:I@ړ‰à?ø»B¶³Ûº?³ðïèkõÙ¿Ø_ÄŠŠ¿å«Lh¨#å¿î"¨FNPSRPSR?ðÐUŒ?4í¼ì›ä?ïHë\ý£a?¤%Љ
	?–É£?t?¤!Bݕ4>۔§0Ì>ÿK?ËQò?ëÇüBaÀ>?Á¿±¬Á?Àß×Î9±?ÁÃ5âæ?'iLlØú?,§ÒÞº?ì*µÁ!ŒY?£±€~Ç~?¼](ir" ?£Gßk·pc?BØ_õK?A="c°Ô?îæyÐDê?•Ø,ÿ›˜n?¡PWš;¡ƒ?•¤R)ì7†3FGL J2030.2-0622@CUv?ø="À8Û[¿CwNÀ9C†åaïÀ;[?ep!?ÈýWlÈÎ@'5·œäÓ@ 6à'Т¿èOÂ)I"7¿éPH÷Y'¿âj˜2CýŽ¿äòŒ~ËY}AGNfsrq?ïü´EÑæ'?AÉ2>;>ÿ®ÜŒ_	?Šþ-ïE?8bã¨"?@ ÷rhDZ?ïÀî&•TÊ?|7‡²FS?SLX©e…t?\¦ÕF
$þ?zµÖŠü9ô?xÈ;J›®Q?ï (»q"?…{¶ˆ!"?|Pt=º¦£?pÂß,V"?"æ˂pcç?'	'…ÕR\?ï¸HïND~?yr•¡xlå?sj°:?@a"'L¨?ÂÁE™€?yYPd¸÷3FGL J2030.8+4416@T–Z?çvœ@ößoçšÀ7«ö©?)À:|^ʐ²j@©'¿šÃ@ã$ð_?ûé/Ï%—"¿Ôd=eÕ፿â
ñ!bGÀ¿èa9çéo¿ï·},¦|+PSRPSR?Oƒ8Ø6á?\ڏ…RKà?쾋ŒQՊ?À*"Ò#Ãs?¹Ì+ÁQJ?À
Ѻ¬ä?1ž~P}"L?Dòð!ÔT;?ì]
ÎZÿ?º@…){§×?½ۂv?º?n"Ó"ú?*•.¢­?{jr°@¥a?ëŸýœä>Î?©bûôîå?À†´âùï^?¨ºžÅ"Ø?I´ö¿ƒ[Û?DoÇ_×ýÍ?îP6¬Al?œÚ†!(?ª•Á]
ÛÉ?œ–'ñGí3FGL J2031.0+1937@O( 2:À'`ÿX±À9¯˜JAÀ;o7…¨K?僧GŠ·@ÇJ	
šÈ?ý5ëˆ"¿ÛãÅñ«_¿©;!ØܔZ¿Øð8^¡`¿Ú·Ñ‰[D0AGNbcu?îp&‡œO?¬u`¼;Þ)?{aaÚ(M?€vÙ#×7œ?¢¼Ñ\A:?ª0«
c¨º?ímhÿ?"…?µçÛSÖò*?†Uê]û?‰D؂±º"?±ÉúėÃ?´?íùÞ,¾¡d?™ªÏ#ü»¢?–_è´ÿ?…öúl?¥Rm?»ÜO?"S
"þ?ힸú1'Ÿ?œ7¹eö'?‰#W»+b?†gÝ$?¯Ëšn"‹B?™Ü1T'·3FGL J2031.8+1223@LÈ bÀ/mÇÀ'áÀ9Kƒg(-FÀ;4ÎAAð?Ô¥}}a@§ÃþÇò@yF÷¶¿ãQßy¹Õ¿åŧ(Zà¿é\1'&ç(¿ÝôÌõUpåAGNbll?ïÞ®®kȂ?plC½l?WmÓPž^_?[äF¨L+|?ešgëèO?g'•±[a?ïz_d£?"Y¬BBdˆ?eÅ'º@°?j7áªfœî?Š0OÖ«?'"ßü?Ô?îϗr"²?‹'Ì›«yÖ?‡¼p¾z@U?y'Ö¬î¤?š.ÙN,Ç?…Ë9B¡?í,^¨¼ØR?¡¬Ômm,ð?qgtí#á?rñ/À'Xk?µŒ"BÊk6?¡' -fÝ3FGL J2032.2+4126@T
ýòÿf?ðMô·ÍÀ6'•¿†À:ª¡(Ú@ðzú;J@
*÷%æÄp?ü†!'Kòr¿¿KŸ:ÃJm¿Ù¢#ÏN¿âmA'3ÿê¿ìY!d(ÉxPSRPSR?Md­³?бZ%òÔ?î½ßÔ©]?§y82
?¤$ë|ƒ[i?§uêóàF¿?!JbÎ×L•?9º49à¶?íÌ("qÜ?®`ïO[àÂ?±–y‰ýo?®c@M?sÄ~g'µ?r¼G#Zª?ëï‡ââü÷?ª>•ßøF?¿Gynüò?ª
Tôà?4IöÂålå?5DÓ«ì<?îgy;? £"{q?®%šèA? "¼ÿù™ 3FGL J2033.6+6309@XŠ?ÿÊP@*þJ`vb]À:k£¢1ÐÀ;Ä×09¿"Þ#õ‰¢@C@1"J?þRa~Ë-¿êÌÀl¹‰¿æ"Û|	ˆ6?–Š-júÓ¿ÖŸjO:aAGNbcu?ïÜ%嗬'?šFÜ\Œa¤?7Z²ÿHw³?K6¦r¼Ð?pwb5dà?šAÀÁó?îäV–Ÿäò?¨fÀR[ã?uÅnò"ƒ§?"_|ß E?žÑobA?¥š
3ù|?îôÂ5}ã¦?–˜ÈYþ?~7uöp?lsƎø9F?™ãkrÅï'?ŒŠ_ʪí?ï m*¡s?'z]²LŽH?=¹mØlÃö?J¡A.ç¬?›‡L£J½?'U`Éü`3FGL J2034.3+1155@L?› 'À0|rŸYÌûÀ9±vfŽªRÀ;wœÏÛ?åŽJݍ©@ÅÆ"8@̵ `]8¿åq¸ÆýÍB¿èÍò¢Ûré¿æ÷£"Šú¿å†>•^mìAGNfsrq?ï¯ïÓè»?—oUÊg?fá6&²?"|¸Ww?|—ß	Lü?Ž…¤½Q?ï_ßú&ˆ›?—U÷‡¹Ó?p͊îBŽX?wf~ׇ5?¡;ÿ<'f?"‰Yæ'?î ÛsCŠ?œ$õB·™?"i"VáK?Œ[v)€Ž{?¤=~¢»!Û?•Ž¡%cOÊ?êì>—íü?²^Øoh"#?ƒ.í®ý@?…gÒ¢Q÷5?ÃÅ\?±Átë#ûm3FGL J2035.3+1055@K°‹ßœ³*À1;`c'À8ihÎör¹À;'ÃbÀ¿x?óÉ®	h4@¼0V½@¾4à1ƒ†¿á'Zr^¹–¿æ†?"ë_	¿æ´KÀÈ¿êAë1^>FAGNfsrq?ïæÛ4" 4?bq/2yž‹?T¿†Ðû½‰?Q>=ÿ
Só?]ŠêÃÚ-?[/A'¢Õ?°Ý?Šé$~'pç?bgÃÌcÐ?fõáîñU?ƒ¡ÙâÕ¡?ˆ¡]ödO?î_™(ÃÂ?•ÃüÏ®ß?—äV¬ÈáZ?‹Uò*ÚÖ?œ(":Ç&Ž?‹Ècñî3­?îõQØ.`@?—ÑUµ‰L¨?eÔf&ŠÌ?f6{¥wf!?ž›85bµ¾?—'>p(‰3FGL J2036.4+6551@Y(¯ ê[S@-ÒA³ÿÀ9¶ñµºaÀ;¦‡dã¯?âG»){_@¯^ìI"É@€-?¿áDˆ¢V=¿à¢8±ø50¿Ó¦ã¬ë¹€¿å‰_ț|AGNbll?ïµÆÚú"Ñ?'CI€€š?c¼bÈïՆ?f‰™Q?{>av­?¶«Æ†"é?î~n(®—?¨°0©_¬<?ˆ{S— s˜?"/´¥K?¡éD7¬ù¢?¥Ü°íî?îå °°¾¶?Ô~©µº=?†ž-–/a¬?{é Æ¢?—üÓÐxX?ˆ¹<˜fÜ?î
#̃+?œó;úíÛX?"ªå@âsÑ?'šUJœs?©´trÿ0N?™åñ纘3FGL J2036.6-3325@#X+€~
ÀA½â:¸cÀ:žƒujæ(À;£Ýs
=Ö?æז(î-<@
–B	òa?ôàÓËr/?íš|˜ì¿ïïrȖÕ?ï¸t´™
?×K;IÕAGNbcu?ï–ý€p¤?£0²~ù?% [֐??ìP7)êÌ?‰ìUt|ñ?£[À~yk?ï¬ä
L?"©tΣ?WäM÷;?|ƒ*‹R:?æ™À£: ?ŒÇA÷6<º?íÊ<Á#ÛØ?œ>T¾ÅQ ?™ƒ(ne]?'5:9‹ñ?¦šŸ¶³Í?"ÚÞ«€òº?î:ߌ7/?²'€Ä¢µL?ö‡Ï?6Ý1}'p?¬Iø¥Ž?²'p

Ôn3FGL J2036.8-2830@/Êœ£9ÀA2¶­À9·'%VўÀ;ªÀ:ñiš`>F@í-–¼¡@ž˜›ü ¿â´låö-]¿å¥F‰Yä¿çÞùÎ@G÷¿çe±jFAGNfsrq?ïì"fµú?`1Þ·2?@/¡´?@«v~Ñ©?^Às±j?^oÕ©U¼?塚"qfê?e(oQ€?SÝ/ RªØ?[†Ÿ&Ur?ƒ5?›ð?·ãªþ)?îüå¬ë=Ä?‡Õ­öU?'<]{‹O0?ry¥'ñ?—E¤ÒŸ°?ƒ¡9d£¬E?ï6gæw3I?åÐpÖ§?A³Î=³x?KC½	?˜ªý'§©?r¬6PÚ3FGL J2038.8+5113@V/×,uª@Ò½ßôò±À8˜ÈQ=	vÀ:¯ÚM¾Ð¿ü"ƒèØF@ŠÆóïÑ_@!ÙŒÂÇ¿è~3•6f!¿êö°Šï);¿èó"ëxš­¿ç·Õˆ¡éAGNfsrq?ïˆæ?ŽÀK(?D½¿<‰ßQ?EÉ­;jˆ?Œ°\†ýÜ<?ŽVÂF19?8{±:?¬#ÒÜÞÞ?e"kö¼iž?rîÅYË-?¤2å¸Ù%Ä?ªÖ?‹6Ü?贏"êñœ?²Ú‹†%G?©ãxеu?œødù«V?Æ´ÿV 0?°7ɵ¶"?îüq‰lÏÌ?–Ɉ¹‹jà?ùð"Lw?4sb"L«'? .êpèÝ?–¶"}^S3FGL J2039.0-1047@A£Rÿ" À<½ÜŸ¨§TÀ8¼äÏøÑ8À;8E­‰:§?÷8(Øîn@£$¨«Û;?ù§´³Pz?§†õŸv¿à:3Ïݛ¿â}zvÒ¿â7è6;6AGNbll?ïsyÒã̞?žïfñ?^ÍëɊFš?iîŒÔAÅ?GÍÍۏü?œµŒ—§?ï#E¤?˜×aïòÝV?x2©×ˆÄ9?xL£µlϒ?–®òiN»?•g.½É#¦?é~ҋ빎?±9Î6í\ˆ?¶G—ÐBñ?£Ä•˜P!?½ÁÓÐ_¢£?©a‰Ð'?êßÀ';çç?°³u†""?•<å4'?'ùzJ|{?ÁÙb¼~]õ?°ÐWÎ)'3FGL J2039.5+5217@VkΠ£¢@
æO†%À:'r—ÍÀ;_®FÏÈ*À7Õñ
ÉÂ@
Z×h\4ß?þGàðñ?ÜMâ'QåŒ?ëHo«¿âP¸S¿Õ¦Ð†73•AGNbll?ï5Ã,'5@?K&R;ð?aW>I㺊?b¨Î8_ž£?—²±ÜàÏ?œ!µ2÷©…?î¼ÑÁdz3?¸|êo[?gErZ–?'Êô8OÕõ?¢¾ŒÇò»~?·½© œJ{?íTFF´sn?žxƒÀ&÷×?˜'~èªv?…žRáG¬?®r\ c½è?š>‡C¸?ïÊè:T?"3!J?ö™?5;ƒ88Š?b#¯ë¡ŽÚ?y8G¯xTû?'¿ž:ì1Œ3FGL J2040.0-5734@u:jŸ{ZêÀB‡ŽèӔÀ:O»¢çÀ;¹Åԋ0¿þî5'³÷>@
ú…\ '@'Ñ`w‰?휃OÄþ¿éó£ËC,G¿Ö[âé2¢Ù¿ìK%99KjAGNbcu?ï¢*ª-½i?M÷à1^ˆ?Y4PD)?fL‡g9ba?"Qnò¦"?«í¥&ê?ï­èL-YÔ?€å†Âi©Ê?RÎi~Ž%¯?WѱCApÉ?',Ä×Æ?~*ƒb‡C?ëE¨"5=•?¦ð°»È"?²I>MÑ?œz7µ£ž?³¼u°üŽ? êú°a~?îÇÑLÂÎ?¢;³k¹Ïˆ?,h~"¸'??lÌòÃ?£f'Á!?¢6sÛ¬´Ú3FGL J2040.2-7115@t2gŸì™òÀAá`xÀ9§™hò1áÀ;†‰1l‰–¿×ñÆ<Ÿ@
Õc¥ì¹&?üÃöM½ù¿æÔcGß"÷¿ÕŸ–äL_¿Ö˜÷f7±¿ÑèP©ï/×AGNbcu?ï¡)&¼S­?‰ØówæMí?C©B£@Ð	?Cñ¡m2?†{"&·K?‰IãTH\?î×£?"IÕü"8[?V^"â~m?W#Øù¦©¢?…ºçúG?ƒ_4¸³?îiÛÀöI?"É⑝;?‹Tˆ´K&'?wîAß»"(?¢!È¥*?'¬íq½Û?î´¤4Ù?"ZIr!??±‹CT(f?Bþe6g›?¤x¢§æ
?"QVO€´3FGL J2041.7-3732@gE_ۇÑÀBš$€	À:w$ú‹LÀ;—œ`ô6ž¿æ«ªùÆÞ@
¹« éð?ü™Þ¸Ý'?ãà¶cÁ¿â·£??¿ä\ÓÚL¿ªwYƒAGNbll?ï'Ôˆ—BÆ?dðÁâ/?9B:Â}‡?9ßõJ{,\?Ž€Ì'¿?UJü£?ï»g2Ȥ}?{hÍ¿S^=?L¦ÆkþA?QÜ䌱%6?~ÈñÂàAÄ?y­+ðOý?îF!e?'\¼N`½?"ñå;Ÿ¼?ƒ¿+}Ò7?¡šåQn]Ä?‰¬œ¿t?îÿÃòê}ˆ?–Þ\¼.:E?#¯ið¶§.?1ÿ3s7z$?Ÿà"ÎÎá"?–Ö•'Å©3FGL J2041.9-7318@t
ÀÓgÀ@Ýn˜K¼À:¬(©lÀ;ɨÛUüŒ?óVµ"ö@Ë$Np@­œ€~Àz¿é«-ˆ×Þ¿ëM‡sb‰s?»fpѓð¿âw ‰s—ãAGNbcu?ïÐܔ=?«»¿ªš8'?`÷Ûá§x?kWÉ`Áb8?šªh8—>?«~£ÐEøR?ïÏ8ùÿ?£k"îÑ?vrjý?ê(_>ª?™ä<Y`Ð? $ú1'5Ú?ê_*ÎF?¬ýÜ/ì¸X?´-ïÕÞß?¡MöhŠu?¸þP¹·ñ?¥³½Ù9àÉ?î'•d°+?§_É­]ž?kEB–…©b?z»ðCaM?«Ùâ€L¢»?¦ŠïöÞÓ3FGL J2042.1+2428@PòaßîèÀ%–Ä!, rÀ9ÓpàÓÀ;†3çÀ½¡7Ì¿@Šþ@8ã?ýß#ÿŽ–¿ëi*Ý4Š2¿Í'«é[Š¿Ôjë%¨[(¿Øb' 4AGNbll?ïï*X"Hg?bt"Ø"—?5
î÷PpÔ?>÷òù`'?\h"›ß?_ÚÑpÖ;?ïyϱj@?™+Fë½<
?^Œ*[<?j÷¼úB?ºµ%Dd?—‹½?ﯪIEX?‰Tì\–?'$¼²1I'?q¹ULpËÚ?"÷¬]¾°L?"eüfJl¯?ïç*Ï-ï?i:ÞL
)>¼'¬'m%>ÓMES03?hÑë;?äI?i7¨v{»Ó3FGL J2042.1+0247@H?÷fÔÀ6ÿ n4'À:Y)ªIëÀ<:&1Âð«?ù)Õq6#(@
É, ð:?áçy©í­¿ËZfØ1¿Õ!÷'"b·¿îOÙGÀš ¿ßk;Õ:¦çPSRPSR?ÜͶû'F?ÓI.ní?Õ¡õ×Æ<Û?Õ;>ê<±È?Ë ¦ZU7¿?̺,
¤<‡?à†úÖQÛS?Õy-z¼g2?Ó¢úç`bù?Ò.ZX>o?ƞ×÷ÌÃ?ÃÀ‰PÀÙ?ގð²å<S?³ý˜À‹?Õäâ'ä-?´W¤çH#•?ȪTÕ¿?¬nT¯g}?ׅÑÉ"<?ÎöþïˆÞ?ޟ9b,ÉJ?Ò/©¦Ü|(?õé¨!Fò?Åü†×ä'Ð3FGL J2043.2+1711@NóK 'ßÀ.šDÀú0³À88í¥,uÀ;I»	Uê@¦óp.@Q	@¢C@Èx»¨'¿×܀"'(}¿Ýk'oŸcø¿à«ƒ½u}¿ì«Àã†PSRPSR?‹ñ{
¤uE?†°ÏN»´?ïS€ˆÚuà?'"q[å?~\Å}|%?}¼^؈?Šªýa;]?'þ7;?쩏ù7t?³3wSG_?·^ ŠÁ7?±ÚaÞf+?¬£ï«º­ ? )¿¨bÑ?ëÛAœD	?¦›¢U?²ÓûH]d?›éü.Z:?°ü¶˜µƒN?£ÕR«ùjï?êu'Ù|'?²ÆÌ¥ð¬…?»W2›ià?©×ø aê³3FGL J2043.8+2741@Q¨¸!ïÀ"NîÀ¨tÀ9*AÖd%DÀ;ré?û1Œ$;¸@dóiï‡ã@4J´RE¿Ö…<6ß\"¿àú¼Ê J¿êia@óÌQ¿îÚâvy¦WPSRPSR?z
rn$Œ?IÍ%2?ïƟ¡?¢@\Úø?•Ãς?žÀ"0Ó`? 	SY$s?œ8ñ äÜ?æ%Ȇ?ÉÐ!cT‰ë?Ò»n©?µ?É5@Ecn?®¥bc>h"?›<0a€+w?êÁçÞÚ;R?§{k.×?ºž׎ñ.?¢çÕ¸¥í?°®Êr4?•>ýZ³?날'†	™?¨.œâîë?³æOù]#ÿ?¢H
×Sï3FGL J2045.2+5026e@V06â—@®k³¤ˆÀ7"S‹˜OÀ:C/(·Ä@¢ó_2•@G™E`Ý;?ýÆøÒ¿Ï©0&Ž¿äùÄ÷k¿èƱ?R¦@¿ìÃ"Ê/c›OTHERSNR?qÉÁ?xLXW¯î‹?íH+vdü£?¸1Nžz?´¢;vº¢?·"—ú†¦¼?UD¡ºC'?d(ºÏP'Ë?ë¯%Â9—?¾ˆWäÇ?Áß³¥'?¾‹|ôÓÁö?—| ²	·?"k·!ž?é|Ï_‹?´¹‰S"^?ÇA£Ô@¡?²ë÷D'3Ô?q{«š9W"?fI¶…Û]¢?ëSC<š°ç?«³`c6ä¿?Â'°Ãqª?«T2ë£7}3FGL J2046.7-1011@Bl@%NÀ>2w"^À:jSâÖ#ŽÀ;"bۗjë?À'@"ɝ@ŒV¹ E?ù¿WAï9?ïðª(¡Î‹¿¾½mÍx¿×."Â3/œ¿Ï$ô'IÕAGNbcu?ïõV¼çì?PíèR.à?(ñ•Da?-8ÃàQ!²?RÃ0"~=J?OÇgX4·¿?ýÏñ}?ˆ–Ç"‡å;?]Žè¤~
?c{ÊÒáxª?"eã‰Ï±?†:€;"|Ê?îÃeÁ¥?Ú?‰™l܍ݎ?z¥¼ÿ½–?šÑ<لa>?†™CgÀU¹?íýKx:d? ßÃí~§?dù!Ð9?mZwŒi^?®Û¶ºHC? ™»Ï­Êo3FGL J2047.1+1054@Lˆ)³únÀ3¦Ÿä6vÀ:\l6‰ÿÉÀ<,)ñk?øyȈÅ`ó@-zØcXë?æʒéYÔ?îËa¦Üi?ÄOð Âv¿à"¥…¾¤¿í¶™£ÄY¥PSRPSR?¯£'ÕÊ?¸b1ÃsP?í$´9õÇ?ÀÜúÉq#…?L7îq› ?³Ïy¤*" ?Ìgíäq¹?É7iÇyÙ?ãg]h‡û/?ÍôÁè×öš?ÆV"oû¡‡?À7`ݤRé?Æ2'Š?³;Û¥Í?æÅÉdôy?·ª‰á80?½m¦‰H(~?§jc?¹™?àlC€"h?ÇÈhÑAmì?Ünò¹Ô?Çôÿ"]²?©8SPêÑ?©xP%¼ Â3FGL J2049.0-6801@tj‹@p2˜ÀAò¨`úÀ:%êIµU¸À;Ä)Ĩb?åæ)Aí¶&@!Úi˜u@xÓ@Yap¿íƒ˜í»ô|?ÐìMë	<®¿â§ým‡¢¿åGqaIÐAGNbcu?ï»Á*Á?­!˜ÎIi¤?e6¹(zc?—žìÒèn«?w"dPyÞ?¡_ ôÊC¸?îšÁ"å?¡ÙE
ç‡?ƒö¹†ìÕ?ú6))³!?¡VcMŠô?œNŸ¥´ƒ?î«[Á'‰f?"dÂԋxN?Sâýj?€P
€*4?›ê–Å°Pý?ŒÙ;:(³ú?í5)u-^?¤¿äìàY ?§äûò¾§—?›Rn³Ý&?¤Èlºorz?œª?Ã?Pñ3FGL J2049.7+1002@LWú€d>nÀ4­€'ÍÀ9=A&QÀ;|v,­5?ÔSÑA@j•pj @9Ûm¿å\'"Á¿æÑX«Eq¿åÇiX¿ç‡ëÕ·¾.AGNbcu?ïä†úʆ—?hDԔ©ˆ?T0y<)?\Ä_ÔE½S?a`øxÛTç?`ûšÏÁ>?ïZ)иñ?•ÂW´ºq?pK{ˆ/Fm?nÐù4\¯­?§ýÃÝl?"^c+."?îø‡Ø[-?‰,¶œ"Xš?ƒýcüŸrŽ?v6î~…Û˜?–ðj¦¤á?'ñ¾Í0|Ú?íò~»ÂÚ?›[ÚÞÅ0`?v°ŽDa»?q¯åÅa.1?®…§šþ?šÜ…	a¹3FGL J2050.2+0409@I·PÿÌÔZÀ8t-݉À9Ø
¨_/À;"8PÍx?ã<ð×v§…@
$*ÌÝ=Þ@‰¨f翕ЉÍô•¿à4Õóo¬i¿ÝmyzÀ:˜¿æÈŒ·€WAGNbll?ëÓÉxbßá?¸?ĀD?œMÖò%Æô?¥öþŠR@.?ºN>€_>?³Tqf3_|?ìPqU(Å?´6Àå_"ì?¦Ò/ÍO?¡O÷''Q?²q
epQ?®¿¡œh?í´xê.¼? Gó"¦.ú? 1ÿå æ6?iã°ñx?­Ò¸Œ<-þ?—PèF¡?çÌDWì?ª'­/EÄã?¯eÃc×Z?Ÿ§úY«Ùˆ?Èõ}njÁÞ?©*Q*#Í3FGL J2051.0+3040e@R¿íÁ9À! ÀŠÀ78IqcÀ:ŠÂp@°1a÷ÁÃ@òäñܦµ?ýÜSûª°Ã¿Ðþ¯¾3G¿ãlˆÌ¼¿åSºÇ犾¿ëÈeÊ_4COTHERSNR?x®IS?x7W
s˜N?률·_"p?Á	=¶1A8?À¤
×äh?À­A»Î?o߉Ƭ"?iûÿßÑu?ì´TÂç&?º"ùâïâ?¹^]¡0¹`?·tˆºÒ?œUå¶?"~xÛ[Ž´?éW•â~P?³¯¢Ò°»?ÇëÕ¯ã?²:g"y¿?'5Do«t?v{Éè£<£?êkäT,?ªZÊ
%?Å-ˆ®"š?©2VýfЪ3FGL J2051.3-0828@C™* dúVÀ>v |wJÀ:yö£•œÀ<FÁƒÃn?ú7¸ék@Ë»O†¦?æ¨Ì]Ÿ÷?ïÿœ)''?ÅýíÍž¿ã4Ìå^¿ïÿMfÿØ,PSRPSR?Æ	Q.?È	,Ë°R?èÏ牤€í?ÌWª÷÷ê?©cTs8ã?·dB|?°ÞRõ3´?µ™Ï¸h•?çî#´w}Ø?É2}{
É?È'§nÄ?ÃäÌ2(§®?ō‹&f?±ÕëÀxøÛ?æC$õ&q?¶}‡ ©'ã?Áeá*A(.?«Snì'_M?ϟÊ8'V?½úv¨äž?æø	 '"	?ÄZÑÐ5Ø?¢nÍõv?¥œ21·}3FGL J2051.8-5535@u]Ø`fÀCx) zbÀ9ÔûÔ!TäÀ;¥°a\;j?ÇÞ¼Eb'#@ã'ÎQ@ž^ qº'¿ë ™¸Md¿çúË¥ÕE¿ÜqtAEo¡¿àGŒ5zW¬AGNbcu?ïûï J?J¿FIR&Ç?ݯië?"Õ¢5—?AÒfŽP÷?I®žYÑ×!?ï¸ü6…'E?€Lý¥g£þ?I`$DI{"?Måü`½?€*ðq—9?~֍÷À~ã?ïS)	?[(Äd?rÙþ'ù¶?b±¢Ìã?é}– œ<?̌ëE"ý?ïˆ;ËɊ'?ƒ©ðªÑ³?(ï(ѳ7§?05vLÂ7?PjV'Î?ƒ—ä–ÓÛ½3FGL J2052.7+1217@MŽnß±«ßÀ4ù@ÉìÀ9Á+KÞ$äÀ;˜†1		?Þ"ɘ\O@
TŸãŠ©@¿ÑÔ¿àÍNnðE¿ãQ'KŸ:ÿå4'౟ä¿äùÿäþ›PSRpsr?åhž"å?ÊÁü<l
?—Ú®îÑèX?–†ˆYçû®?ÔsƒÕ×±?ÊC/õ"UŸ?ít»X¶=4?¸Í›0H_ß?—iñ†ˆb?œ'L€¬Ï´?­+•{Øè'?³†èßäá?ì0(áþL ?§Œ¦¯Ý?ŸY<ŽÏ?‰Á´ðaü?¶¼âªþ{8?£KìÌÆ?èI…ÝÌé?­;˜SÄi?ª§âI#?ž÷BÎ7?È/ðýk—?¬%ÒÌ"½Â3FGL J2055.0+0016@H9Ÿ C×ÆÀ;
v_Ø­¬À:xÊ J"cÀ;ž‰.‹C?)ÃZ<¤c@úׯ~Þ,?ûºb&%Ú?ïô>!gž¿èþúÔÇíë¿Ú°à¤a
¿›K§7µ"AGNbll?ïÔ>3³Ø?%P+¾?aƒ•Ñd?%4|[™?uo`¼¸Q?UÉ4¤?ï³^ç"F?"÷¯œsÕb?V<ón1|=?^
˜Éw³?€t‰ØX¿@?ƒkåCMä1?îÅA­¡­?ˆÚ‡Óñ–2?…UU?à´?rwîD@?œ‰¡<š3?"Þ¥Â.iú?îa2ò-ž…?ŸÒ/—̯?:9•ìU?PììçÃ?©¸]±N?ŸÍ´H[B3FGL J2055.2-0019@Gó¢`¸À;hT`ªdÃÀ9ïtŠ˜À;cÌütð?Ü —8°•@hcJ?ùÿ!@AŽ–?o=òÌ¿¸íý^C¿Ì®ÅG>пÓm•¿ÅRZAGNbll?ï½n­ˆ»\?³¯¤Ë?OÙcƍ{?Xë꬟ñB?}M|ÂЮi?€1'¹«ÓJ?ïâ'¤@?ŠðŒ> ?cEri5áG?gZ½âð?†ö|²7¬?ˆÇP½é?î"?Hú˜ž?'ïúm?Qñ{ò6ë?~Óì.®û¢?Ï"³Ð¬?ŠÞSúÙòû?í#–Áô?¥ÛNèfÎ?p#;HÉ?u6Š²ó)?µáÍ>ƒÔ?¥ŠÒ¸\P¤3FGL J2055.8+2539@Q¬iöZeÀ)
¼ßÿ«À7 Ž]%uÀ;=¸·a+@~ÃS&m¨@JԏŽÔ?ûÄwÌk¿¶ÖĪ5ël¿ßc–éÍè¿éñ8‡¹zé¿ïÿÛrW
~PSRPSR?R¾Ð¬%z#?Z÷'H{?ïÅt¡ÊË?ƒ¿ZB±›ù?x•û;Ø?'X±áá~†?=wu–éè?U÷ÎW4è?îÃaz·—?¬¾µ˜Ä2Æ?£ŽùisÈÆ?¬£ˆ í-?›R‰%)uÐ?'Ö$ñVÍ¿?ì"ÿªøg£?£Ÿ±.kB+?µ`^òev? )ù
9?&E—§å«?*àÞÙ¸?ïÜl•r7?pûYǜ Á?qˆ¹‡»Ú?p¥7éŠ@O3FGL J2056.2-4714@v	k¿×ÀD0½ßÉÿ"À7HErÐ×ôÀ;|ê6j?ûü%íûE±@2ê
$@©³ûo¢z¿áO,²]r¿æ㺠^Ö¿çºg΁"û¿è;¤=XóYAGNfsrq?ïæqí0ôÏ?nÅ­dÅO?WŒ
"0x?VpÂÃøÞä?[V"ô5?köÔí¢Yx?ïÄΨ9áž?xq£ÉŠWj?HBñí ÁÅ?M7oê'b¶?zM¥kÕ?vŽ°!q§?î»A2@a1?•£&ºbð?'§¶˜±?ŠÝ,r½'µ?–†2©=AM?˜øÅY£?ï×Ò`ö­±?€ufݔwƒ?ݹQ‰•?0£­jŠª?s›X oâ
?€câMÉb3FGL J2056.7+4938@VSI`0Â@@ô´À;™ßÀ8ÖéÆ×qÀ:ågÉ<õT?é
"v"ÜÆ@[uLj'?üˆH€ø8¿×
Àي±†?ïýmaw¤¿×:CÀãϿݨSíN2ÏAGNbcu?æœïo@¦?Ç{"~Æ?µùÓ5†z?ˆ¹Y±öÊ?ÑØqRå4€?ÇKÓt
?ä€Á"̇?Ñ[y™œ2q?¼=ëýƟ?À?¦âÃS™?ÐÓ¸ÖõJ?ÌùÓ±–êý?åý"D•±–?¶vÖ.'¡?­¯2«E?™ù(MH·?ÐN÷ÎGk?´9!5Ayû?âT÷,ÙÞ?Ã~¯¤Ž™S?ѕ®gº[ë?Âљ;c?ÀÆ}#Ïß?»"] µ8¥3FGL J2102.3+4547@UÀÇä¡Ö¿à	'€4\˜À9N‡"žyÀ;˜áãµG?ù°Ñì~@¡/Æl5ˆ?÷Kc-vÛª?´  S¿ã¯¥$W¿î£#á[¥¿é¼å~tz%OTHERNOV?îsÞ¸JÁe?±·$š?…¢©
ÜÆ?¾*¸œ1?£Y'Ñ2e?¯BñÊ%¸'?ÝߣøW?Öþ´€:À?"5"´'?`? ÿw9Û?àÏäbš{?Öº©Ø©''?ã®S‹›Õ?´ǖ(½à?Í%äŒÎ?°âr|-?Ä "Dª?«2ÛÖ?ïQS@6ù¨?—¡u!Òôb?pwñ,Ùe?€¡$Ðܵ?'·ÔüՔ‰?–R-×EK3FGL J2103.9-6233@tË¡ ÏÀC{+ŸÀûÀ8è_⾦™À;em¼Øc?é90&³Û@Y–ù+O?ÿ›I?2É?¯Lùû%¿â¥—\[(M¿ÞLYy1Þä¿ãEÊ/ŽŽAGNbcu?ïî˜ÞæP?`qæŤ<4?4éf­m?4ÒÒÝ?]ȹu´¾?^›E€ƒŠ?ï[
¾Î?'0`:A†×?g[ÂíSÉQ?i5|P%ùÁ?'¢¦J{¶­?è´—ˆ?îŒì‡†Kþ?"±áúhã(?Ž¸B 6?ƒ³>²<=ß?ŸXã³0'?ŽÃò"
ÑÜ?ìqÌÔ&V'?©°wƒh–?€ÍT»6?\œ•ÊU?ºWõÎâ´?©2~ƒÔÓ*3FGL J2103.9-3546@aåéSÀD³, zûÀ9tÀ#i'À;§ò¼JžŠ¿Û÷øYÃjÎ@wçî@ç@GD¿ç	taÀ¿ä=t:ö‡¿ÛJÝQ‡å›¿ë²æë´×AGNbcu?ïå[Ïz=r?mÀ½ƒAÐ?PŠË`"Î?S¥'qi¥¦?b k |´?h×䳃Ü?ïºAª²½¿?}Ö;ÝN¶?O|×¯Q?TQcÃæ|;?~ïšk«<±?{a!ÏØ?îD½z
IÐ?™@ÐÝ.½?œ¨‰Ð¥ë?'ç'MÈÔ?š¿ÆîÚß?Š^î¤N]:?ï«oOÖ³?z5®Ôøõƒ?"Õ\K•Ú?(#Qï:O…?"Ø׬âÁ?zFûP93FGL J2104.2-0211@G°l_¤«FÀ>Hï 6kÍÀ:­ƒðºèŸÀ;²/ãšj?èÄàåç·@$+"Ãyg?øbIÿ''ì¿î86#	ð?ï²ؖO?ª¶Í±ú
£¿Ê]JÚùòAGNbcu?ïóöœ2?Y~H6~m?5¡L7J?<ƒ™âªéF?RҔtã×Ë?VDÍR7l·?ï\n´V|?˜sŸÌz?m¨Xúéò2?xmm¯#?½Uвd?"°ϼ÷d?À:?'
%â%*Â?>a21ë?7yæ+j?œ^.ßù?ŒO•#ü«?îãÙًJ?¢HXî"
?€ƒŒ__q?´£üÕ?›CY^žæö? \që;1N3FGL J2106.1+2505@QðMÿÒ³—À-\n>¡ü?À:íA·ZuÀ;âž43?ØR‹!J—B@žo}¼Ch@8©€—j¿Ú‰`&x:¿ë9¤@^p¿éV/3¿Õ€ùŸ¾¡¼AGNbcu?ï¸C6¡|?"Ë »Ÿ?mØH'O?qcÚeòlu?tò@›ÀО?~ë'ÚÜ% ?ïDÉ2"|<?¢¾ú–ÉŒŠ?tl Ñ¶?"õTˆ`?'K²E<3?…‰=À¶?íõw7	‡?•Â)˜ob?—¥¡«èÃÞ?ˆðçЫ#?¤Õ»²•?
B®C€?íî¸íEPÖ?¡~"ʍ¤?sëd ø?ztÓ[ÓØi?®—
ˆn{? ãiÖBÅ3FGL J2107.7-4822@uîâ@1HwÀEéÿãzŽÀ:Ú
'/ðÀ;ª¢år¶¿È¯!²x@d
"Íڔ@°vÿeÑ@¿êÎ+‡ ÑO¿ëyµbÛ¿Ûý裗õ*¿Öû%¢sTXAGNbcu?ïÙzœZT?'y'üáïB?!iJ­¡!å?@'ŽÔ|º?r·¨\eÌÍ?'üU9ú
ç?ï¨ÖÛ ù?‡7z$Š+?RÑg{i?bœ1Ã~v?ƒp(a8ç?ƒþKæI?îZ¸jØöÇ?"Ë̓ؽ?…¹ÛòvWu?s)ˆ´|	z?¤æUÒýÎ?'¹m—©úÃ?îâë1í'?";Ge™%?8	A'I"ð?E
=ᆞ?¡¡:k¼"¤?"/{èn2‰3FGL J2108.0+3654@TF= ÿ:À،` &;À9ûì_9K{À;8Ò¯dÝ?Ú£D¤Zú@
ŒnPzÂ?þñæ­j1¿ì¯ižª%¿Ò
ØznÊÓ¿Ò8ÁS-4Ó¿Ýäî–VAGNbcu?ïvâƒ?"3sïÌ!E?TÂ+Lž/?UËi>_IX?áBç^?"´u!??鋯>±7?ɌϺM?˜LMËTÕ? Q"Õ…Ÿu?ÆǺЈ?ÇC»¡Þb&?îs¯mlŒÌ?""F¦'?Œïõ—Qhû?|œyr=|m?¡‰ÃbØþ?'$Yfµ?î*2‹A{œ?œ4-J¹Ò?sKúZoÜ?xTtf‡Ù?ªù
̜øF?š÷ºh@¡»3FGL J2108.6-8619@s&¥?À	pÀ=)¿"å­À:¯º¨¦À;Õ"[tšÝ¿ë÷>$þ½
@|É®4[Q?û×à3¿Øm1Vd;¿è—t¡mN¿í§Ðë"6Ë?펨¬S|÷AGNbcu?e4?'Êð|];?SQ¸{쐍?]sËIé²?…Óåê©!8?'ŒªlïÌ	?ïÀX×e½?†QÞ57o'?Tø—øѲG?w)‰ÊWSŠ?z•n~˜´Œ?{p«u¡•?íVI7N?…¾{G‡I?¢¥=+y¬¯?—"¥ÿ™ô?§úq/òÞ{?"vjÝÇSÆ?ïÓÈkž?ƒ+¹'">÷{z´ÒQP?ù¼Í8ê?v^õ¡^?ƒ)Ž#í`3FGL J2108.6-0250@G±$€	À?"›Ÿ-WQÀ:6û>ÐÀ;á3}]?à{@,Ù@
¡nŠLI°?ÿz 'z?îÖî&
Û¶¿ÑùÚ*Èy¿Ý0°ä+Ž¿ßF³u/NoAGNbll?ïѐ@r?qLÝE{¯¤?Q,oH%y?R䟶»ëH?rìÃôñ ?oÊXÍÁÎ?ï7wàà‹¬?š¿lÇzä?r|ŸéQ?yä@zn%!?"qÜ'0?–Rd|1>g?î¡îná՗?‹ßÇLÔ?ŽêTȼÌ?~Í[è:Â?œM¿·îÈ?"Óè	7T?íN »n'?¦M<?T?ŒŒ#T¯?ŠÀº:—·‹?±ùy´ ë?¤Êª¬ÀÇE3FGL J2109.1-6638@txYÀe¶=ÀC"ÿ®¡iÀ9‰³Ò*àÀ;ª'	±¿ÔZ䯘ñ@Ô×cL@´ 06ª¿æÀøùÙþ¿Ú"Îl›E¿â;ŒÊº¿à–j»­AGNbcu?ïÚþS%G?ocM—§¶‹?C‰úíä??Ó"ži‹n?pµôíþ…?mÁ÷õ‹šÏ?ð" ?…zCÁ]º?U}Cq!'ê?ZˆÇXàb?†îÛmÏA?ƒqú(ú?îæý<?¹G?‹®ÉVpñ‰?ŠFªVÏä?€xùE|l?•ýt]o?¨¸¶P[?îô•xnr?÷smÆh?Rš '[‡¯?SNb>"ÅÎ? !ÓuúØ?…•9~W3FGL J2110.0+0812@Mş±áÀ9׊Ÿb0À9(µ)B©À;gS˜-ˆÏ?냚þRþ@3N5m=@š)€Výh¿ç˜õªf›j¿ß'<ä{®ç¿ãÐJÝ7ÂÔ¿ì†Ð¯ÝAGNfsrq?îé€@‰?šˆ¶ÆÝù?§ÎJïJû?™ˆIïXþY?t ¾F"Ê?q$é3'ßÐ?îÉAEL?¡nß©=ü\?ƒµUÒ©0?ƒy–'F?œý,Á
(²?žF—‹ïn?éj€å*?¯wwAñŽI?Ã#õsvQ?«¤ˆrð
3?¬É¹Ø߆f?˜ˆ˜Ÿ'=Â?ì¥'Q¾q?¡es 8¹ò?™É* ·BQ?~gH­Ï?´dzÉáCç?ží¸Ú@Çý3FGL J2110.3-1013@Cè
`:Ó;ÀA·q?Þ<aÀ9™,å;XœÀ;˜£Wˆ}?íjìÖ±@íÌR(—@±íӄø¿âœJ–|-οì‹ßG<™¿ë,•yT¿ïö©¤2-AGNfsrq?í"…"°§Î?³M

&?¦?BLä;?§»é‰‡O®?§˜kE¨žá?ª…­ÄÖ:?à›Ž
ÆE??Ç;N£ÂÄ?Í­*	#Š?ηÛͽ?ÏäËÃçx?Á;gÕ³:Q?é×v÷-áç?¯Dûò±?¸ÖOÄ0È?¢Ìuˆßí5?¸mø'}À?¢…´ã)í'?×Y-hMê?´z}
£?Ø?Þãï5?¸ZÛDhñë?А'¸Î&M?µ%«°-k3FGL J2110.3+3540@Tå€!ùOÀ Éî E>À9­¸¨RšÀ;kŒñëjG?¨—VrxNŽ@çêô€@(WÀi ¿ä¼ó¢	æÅ¿åû§":´Ô¿èþ8
,Ñ¿ïÿv¥NAGNbcu?ï;òC'Æ?˜W–
_{?7k#+ݲ?r¾AµËØ?"j¦îįñ?•÷Ér?磓¯ï?Å˙m÷?­ðÏM\	D?«ª>I¯…¥?Éõ}pa?y?O\…±??ìƒÝ…#YQ?£ÅjúK?«ÅÙþÕ=?™®Jƒ6؎?«ýÓ˕­?•ñþ‹)™?銫w¦}N?ªîH-é¼f?ªý5K#;?ž§ÇeD?ÃΝIý?¦5h"ݬ 3FGL J2111.4+4605@Vy?ò^W¿÷v•âHŠÀ7ÙôŸy­kÀ:ÔàáVǍ@›}¸èi`@©€`7£@EÓ¿b:¿Ôqeóп۔Îs•ùÒ¿ä$Ä
'f¿éÖéë¸í"PSRPSR?'2˜²™ˆN?ƒñ}B¹Û?ê.¯æ®ç¹?Äi?›ª-S?Æ"ÚȘ?ÃäŒGíøÏ?.˜{vZ?9;'´ˆ' ?狔ñIæ?Åé‡óA¿Æ?Ðç#3ä|"?Åê îþ?ÄóûB?¬X¥Ë›
R?à'~Eõß?º±~¶'Ôx?ÕK20z¡?¶"»Z†°?"Y58+žF?ˆ!Äãyy|?ëVR׊²?­@^—¹L?Àú҅m?©ŸQŒÑG>3FGL J2112.7+0819@MZqÀ6¼UÀ:OoŸËÀ9‰˜ð&n)À;b8¤Œ;ã¿Á"^¡\@r¸¥š"?ü昛ü ?݋ë¨|'Õ¿ì®w/?j?Å¡(†Sc!¿Ýæ×½
3'AGNbcu?ïыŠ: P?"~<ÞÀ?.¿½_žŒœ?1~ŒK¤ð?vD<÷òã'?Ï­š¤?ï¯S?c|ª?€ç¢v_«ª?Xà¦@g³ž?Zw=ƒ_»ž?_ßJ?~\êçhP?î_ìº
Í?˜hd±?†"#Œû¢$?yÏüÄe[?¤kQ j•?•Ê.¨]-Ï?í¾°Ö0¶?§"õ?Î/Í?'PVxÿ?9«pB@o?±þê&k#ì?§€øد3FGL J2114.7+3130@S¢åx•À'Äi¿·:"À9ÿôU§ÒBÀ;† Ô÷=º¿úÂc·àV—@Er•É«Z@ʺŸÎ'ô¿á?+¡Ä`m¿íñw³Y¢ø?Ù"V³¸¿ì¸ö´&ãšAGNbcu?ë3R"4ß?'V¥œ$?"›¾{b@ý?›rT.'rX?¾Ïu̅ÈÂ?Á¦CîÜÝ7?ïTha[?¡Ñb¾>á?g@ïñû‰?r'†Û/Çt?''Ë¿V^O? up»ÏRË?ê[Lç'@?¨øW›—ºr?²"ØC{«Ç?›'pŠ<?¹âMUHB<?¢Ñƒ¼qó?á¨ô?®±¾Ÿ3?Šºgî!?5òö1?®º.ôÛ<Õ?®j­œA®3FGL J2114.9+5448@WÁûbâ@'ßÕ=4À9Á¸øÚqÑÀ;ÉÜCbU`?ø½üë"£C@·\^¥§Å¿ùÄ™€í¿ÞYÀw÷)忲o¶*ÁA¿Øђ©æBë¿îiYÙÌJØPSRpsr?ä/¼ï;¥?Ùeô€˜?ÔΙéUcd?×ÙàÂՆ–?¦™Dæa*'?º^ˆ™¤?‹ ŠFï?ÎߒÁ0?Ü&£ˆñ?Õ k2_à)?ÚÕ§ŸÚ˜?ÔX7…'Ñ?ÈpIfÿ<ç?°>‡µø?å&ښwê?³?aTM?ÂôL/$·s?«éG",?Ù…ûˆg"?Ó01)"?Ò'¥Õz÷^?Òô`)Wë?ÔÔ.ü¡?Óå6'¬63FGL J2115.4+2933@S'"Àh¡À*™egÊÀ8ÛN?(3üÀ;lw—|?áNø>ѳ"@ʱ…¶Ÿ@û
_d¦¿å•´|ôÈ>¿çæb3Ò¿àÔ¡Vì¿Ü]™j#AGNfsrq?ïØÖÎï¶á?psOw?DJǶš¼?@ÅÖÎI?q?'aÜ?p9Ž"˜Š?ï	ëНêv?¤†Z"˜?zd¶×1˜?‡ôÜ%-r?˜)X6_dÃ? Ësã€?în
ÒBd?—±Þx÷R?Š_WÌEh?~†''ŠLc?¢ˆ_ʗ§?"±Ð^#?í—†–??¡õ«~ü2i?tD9$I°?wy§¼YÏ?²Ø1{Ã8?¡]¼øáH¼3FGL J2116.1+3339@Sóˆ` ÒÀ%K@¡À7ôò3Ž£À:Öøp¿…¼?êíª2‰b@AVóרž?þ"ëßâ~:¿Ù@Müì¿à‡Ùí`"ê¿Õßy¬X&÷¿àŸA=%êAGNbll?ïàþ<FA?m¸®^x¢g?"û@›"¬?#Ӂ®V%%?nŸ°H?m!D¦4A? ÜÁ?í_æ¼cH?]©æÔÃ?c7‡‰	°!?…áÄûÕ ?‹@(?îú?îy¿{è?™&ÕçG?…;âá2YÝ?}L	"ö?£—"à¶?•Å`·¦ÜÐ?îõnn¦ûE?'áÚ@ì‰L?4§xHÚ;Ê?B>¾æþ? Ê$þ—Q?'µæ™¸Ñ3FGL J2118.0-3241@(üT@Éô«ÀEó; g~"À:BÌ}À:æÈ~‰rÛ?ۊÒðÄ@
CùÂ#P'@|#ꬿè­Xíú;g¿è`"·"Ò¿àƒŠÚË#f¿Ùq·z!¦AGNbcu?ëeÍÿäØí?Áƒûpéi?U6ŽÌžM?aÊ­¨ò¡ä?Â>ZâÔq?Á|rƒÖg?虜R4'P?‡½$þτ‹?Rï±Y²GÐ?fnñ'Öcæ?"tuG¿ã/?"#—5É?æS7o»7˜?¶qÌ%?®¥"10ó? °"¯^<ƒ?Ï	Ù´Ñ`?´ÁÏx£B?çdoÚi²£?Å9Å"Ä?bßGùn?wߘ©ÿïÌ?ÑŒzÈ?Å*›ŸæK3FGL J2118.4+0013@Iû
ÿ±À@Œ@ÃÀ:Œ"\BööÀ;ÓáYKË°¿âM4CÝ@
Ž°?ÿ_@wÏ?4…¿è&Ÿ«Ÿ¿ØÀúýÈÔV¿Íô÷×E)]AGNfsrq?ïúó.m\F?ECæëv)?9bK¬k?}VV¨.?BQ²´j1¤?CžçŒn±?ïÇ0
ï?w胊«Êæ?M–¼lŒ?Tg'¡S~*?xµ"úî
C?u=i
"(??ïST‰ï8e?ç†=?xä¦j†±?eƈ³zºd?$ë0ü£;?{$'8Ú§?ï¡Cu}zß?ƒèEŒÕiE?XÒhÏ?úþ®ÖÒå?‡˜É΋à?ƒßh[vâ3FGL J2119.2-3313@'›ÙÀÑÀFê jšÀ9ëãïÿüÀ:ê ;ꊿè6+±<V%@ñ0¯J@ÐÀ¤ ^?îtXûLo£¿Ø	2åk»K¿ì1Vë…ZÙ¿Òàò¹pyAGNbcu?ë; g¿?Ăû] %{?¦€—«P?ª£˜ð{
?¾¾\¡Ï8?®\ùµ™?ï¾ú5F¼á?"š´"——"?P2¨§»p²?k~`Ë2åA?|v;2²³á?DäùWH?æXàÇO¨?´Ïj]wŒ?¶]%NÃ?£eŠRø?ËmíIÖµþ?²éÈ
(ð?ë¯?(?µ·!ú¾?SwáUû—³?]Í2É«Bn?ÁØ0?´ò,¸•ay3FGL J2121.0+1901@QPàÑnÀ5A/¨;ôÀ8iÎÜq…~À;FŸù/+g?îrIƒ#,ø@J»Þ'òá@DŸWž¢¿à‡àUÆ¿ã0ÅDÿàã'æ&]¿è¹;–
)AGNfsrq?ìt'ûÄ/ù?´gô—ÝŒ?®ø³¹0´?¬™]ìöé"?ª²çϹ?§}u¦!o?åG?ÔvF?Çû˜ö)§?ÅáƒÐ´Ý?¾'Ák*';?Å|Þæ?¼´¡dèm?éø %P)£?°fñYIùÍ?²*'üûU? Ó"ØFè?¾l؃]å?§çlÉyÚ5?âÒëŸÓÑ*?¸àéîqîž?À'o¯'OQ?°–¤I¯?Òp菶?·pIÛé߄3FGL J2123.6+0533@Lüa_–hÀ> KŸ:ÃJÀ9í.÷<À;®á?J˜«?ÐU5åGËy@H°Vï¦@`_ÂWÿ¿¸
PíПã¿åk\¨U&׿âGÁÌ#ë©¿â<I}³›4AGNfsrq?ïÜÀkä×É?s[žf¢?9G"Byg?7þ5å'æ»?pQÌOô€?rxVð!6¹?ï'ó¯Î+	?‰Ô©ÃX´®?^Ú
xm€?_k:Ǭ9?‡gÒ½g²?‡û÷ÝGâÅ?îÏ÷Kë2?"zݧ>?‰g^N®ƒ?z»A‡"?™MoÏ+"?‰¢w	†¼:?îd$§xh|?"–D½'`Õ?e&›*RÐ]?aOùn3N­?¨kKÕÔKD?""§7o3FGL J2124.7-3358@%ß# îøqÀF¹ÿÅGÀ7õˎß+À;MÀ‡D,€@ªaèÓ>@Käÿ¬ä?õƒ…UE¿¨¨ƒþc¿ÒPòÌ:֖¿ä¨‰{¿ï"å™ç+PSRPSR?j¢2+ĵ?yƱ•
à²?îyÒoúô¾?´2Ý?¨}?¦¸µÝ"s¨?³Yó¨VB~?q³	ãéa?…{%È×J?ìÙÈ7ð?¾H4YÈð?¸%~Ž¸ç?½™æ2®?r"U $?†Ý"GrÂ?ìyþÛ&¸?©ÅZcIE?¸ÂóÞÁ6?¨Û´Ea?\?ïÐ'3?W°?Ԁb?ïeKÅ¿Æ¡?ŠÝj;0Ú?''ˆKÈ?‰Ð_H]9ú3FGL J2126.5-4605@všßµÝÀFÒf€g™lÀ8Fo?Rü&À;….0Dk?ñÌs)˜U@nšúíœ@¯àÄ¿âúz§]sñ¿çžâ¶:††¿çê^¹ÚèÕ¿ëøSçïÏAGNFSRQ?ïë®ÀÂx?Z_/]äj?OG=s+?Kåauyå?YCÄõ9?SØ;B?ïÃY'Îýé?|Î	)" ø?H€˜!F›œ?PwZǾ?{C#"X8?zĉpU6?PIœ?'àªDßÛ?•.N…s8¨?†PBOÐXR?"|'ql³½?†²adÎz?ïØúý 9Ë?{Çú´™?'UU4ÀÒæ?1þ´Â»ç¦?rÇֆ=*?{l*öH|3FGL J2126.5-3926@ú'À9@"ÀGÅ 0!0À:^
ÒPšÀ;ç;¥È|?Ýv­©ÏzZ@
eWСm£@ŸÔà—"ì?ëíÏ¥³òû¿á
§ù®­'¿ß¡¶{%Ò¿ïÿuQCr#AGNbcu?í×cH7:Œ?µaüڑLì? öý—1< ?«rµª˜"?¡'Íå[?«!™\ä+?çx*˜¬á?Ȕ1º¬™î?½t ka?¿걨V?ÄÐUg›ø?¼žªØÏrk?èQöDô—Æ?®TAÏ9ø?Á Ó2)GÅ?©'³ô ä¡?».§t²C?¥Û@.%U?åæ³àK0?¾Á½%Dç?Ä<æ¥â€?·º—ŧ.?Ç£~°ØðÂ?µ_"C+4†3FGL J2127.7+3612@T֟ŸØwüÀ%%ó_ÍTÀ9\M}À;DÈ6eÛ?㛽®CA@¼¿ºÀ…Â?þb±Èd¿Úè—-®¿áDâŒôçë¿Ô©fK
šr¿Þ"%öx†"AGNbll?íæù*›?­ Ÿì'"?vG¿Û¬î?w˜l»y?®ÇubÀÍ3?¬DRAßg—?ì,@‡Ég?¾€W ¥›?"yeA6V?š
fœ7(r?¹¢qPúV?¹ºíytŠ?ìÜ£´S]?¡ÿS£Í³? nnzó•"?Ž.Øߑ%?°ã°ŒãšT?›©ê½Ò?ê$L§ÅG(?£ÑP9á?‡Î¦^Îý?ˆŽqØÂoâ?Åñâøôöj?¢¸­ò9o3FGL J2129.6-0427@Hu9ÿÖ•ÀBsÇä¡ÖÀ9G¢[	;À;"ËÚ^†?ôß»6¢S|@dëÑëþ@½' Pˆ¿Ø]:vQ¿â©'…UêÿçY¤4ŽcA¿ìŽËj!0ýPSRPSR?ÒÑGå4ƒ¬?à µ>GY­?ãQ;?ÈC?ÇGøåRY?º2'/¯<?´Rã>›9â?ä/ôC4B?ÁÿÌzs?–ÂÅ«¸5?»ï]<<>ö?Ì©l-ƒ=Œ?»ÏXO'V?ÔŸò.²³?·"`4ŽÂ‡?áøÃ,Ô?·ßOæ"È?À´òwI?¤e­Gç½?àpY뜫?±S+1-"?ÓØlü=‰ê?°î‡ä[Ð?È9dŸÖy'?°Ÿ)ߥ3FGL J2130.8-2745@3ÿV_ˆ%ÔÀFéaÀxiÀ9àwŸsÎ.À;¾:bÒ]?ðÍB"xm@
£*ƒ6UÒ?û-_ÿÄñ·?ï:ÀÎÅS?íãqàÃr¿Ö‰í›	Â]¿áoxæñ'AGNbll?îÁ‰¢(?°cÞõ6
‰?zHIEÚ?ƒ^Îá…=?ªÚÕfm: ?®\±,?é%&äìB4?ìi‡ß?´?·îkxï?¹ÝüCވÝ?¾èH2um?¶¿ž•Åã?ëi7°CÖ?ªõ/=›?­s©
J?šqë®Ïˆ­?¶2©b3'?£(ªa?áڜ·'êŽ?Å0±n+?Ö!(÷S0²?ÆEÀŽ5ÎÙ?¸¦vf›èÈ?´ÜO•>HF3FGL J2131.5-0915@Eòp_äl&ÀCÕQßƤ•À9^YûIÀ;…¸¿Þ¨?Ø´öp£ðÏ@߂ÃiKÉ@1ÿ¦™¿ÜVÝaÅlÜ¿ç€À¶F¬¿ÛOt2$¿ÆW†àÀ†AGNbll?ïØš'rt?uAí2ž§?=`"‹å½?:Þ(âŽ5B?r©w.æ?tÏz£¸O?ï¡sè­¼€?‹xü[Vá?U[âçw½é?e!¢>Îd?"÷‰w¡è}?‡MnîÞ?î¸BOÞ)ø?çþo%¹]?‡"5¸N?x3 öJË?-öi^™ß?‰8BIá&?îcˆ±˜í??œ;ƒS@À?O¯‰À,8?_>÷MÒÂ?©H¶¿o/j?›Ö8÷»Ê	3FGL J2131.8-2516@7‹yœÝòÀF½aßîèÀ:C(ǀÀ;×>â"Þo¿÷Æ<lí¿@´Ô©˜@ÿÿ&§¿à¤\—ÊP`¿Ú§Û%Õý¿â"Ò«Å&v¿Ü.ÛHP7AGNbll?ïÕâXÚµ?qÁòl‰ý?4­ãÒ?½?5rJ;þ®þ?sÄ´½î?qZwJZUß?﷍456³?~I¢~‡»?Jv5´"?P‡sY?€uO—p2×?|]¦ë$5Ä?î=º®%ë?3çHq4?·v 9?€Jp¿#Š?Ÿüšµ"?‡ñývòB?ïšH1®?€(»­Ndž?Q_\¶?ÔqÎdÜé?‰GQ–Õ¿^?€çr³¦n3FGL J2132.4-5420@u]8À>-ÀFqEÄÁfÀ9Gíf H
À;·¢šÊB¿ë¾É e@d¥‰çÊÕ@X`"?h¿åÊv''²¿é´ìӟÇ(¿á†1/D^¿ëˆÎé¿7AGNbcu?ïõQæ?\%/«Úh?!Qs±ƒÒ?$†Î<¬?S›—y+Ò¦?Zô?a2Ò?ᄃ[Î^Ÿ?ßj—ã]ö?Jæ'߬²2?V€&=ˆ@?}OÛ?|é¼®?ï'ÑÝ™?…½uVž.?'ƒtªù€?t'Kµþ4µ?'Ì‹x‡Œÿ?€c??ï¼¾Ãà5®?{'Ô‰Ëf?Òá! ø?"»€8*¤?€¤ªþ0RP?{fO"U›.3FGL J2133.3+2533@Sy?ò^WÀ2ñ1Àll:À:IÑqw<À;¥É¤úì¿ìþgƒ¿4*@
Ÿ3«S*t@çU ›¿ìxÛ¢S¿×gb!sK¿Óþ;ĕ¾¿ãÞ
ùÇñ`AGNbcu?ï㶵¢h?q¿ÃÈ6=?8BŸGU?Ak»äqù³?iA˜ht´ñ?ouã(ᓫ?ï¢É¸!P¨?‡YoÄø|ž?_,t}²h?cf"(&'ˆ?ƒhgõ"°?…@@×u?îñã"÷h?Šcé'<E?"#P'u݌?szн¤w?—±óXbD)?"÷<X‰ö?ïHó"@*^?ˆí_Ρt?,IàTfÓ?0¤EÚÈxf?–¨ù·QçB?ˆÛàŸä¾3FGL J2133.8+6648@ZLhß½jY@&5Á'ì¯À8öüšòÀ;Fçž	jãÀ»zgODŒ@·5Œ©Ç@ŸMÀ¨&O¿çv\{è¿åŠÝì&PÄ¿ÅõJç¦9¿Þu&HÐ9¥AGNbcu?ïù†òÕ?Vß¿U~x?
‡…¯òÖÓ?!oÔz€?H¿8õza?U|;ÇF?ïÐ:Ú¿Å?«îÈrj?aÊzù"(?nK…Êê6?¬©Eu'H?ªeµ\{gÂ?îÏ®	°
?"VŸ°
?~™:2Ð4ê?w#Ã<˜-Á?žcð=JOy?':žL£²Ý?ïèÂ2N²?hs,Eq>ž…64>¶°jü"¶F?g<مv¤î?hq²õsgd3FGL J2134.1-0152@J3lÿݛQÀB>Ÿ¾vÉÀ9ÂzcÀ;‰Ê)"]È?êåúr¹9@_Ə@¨õ (š¿Ûk–/§¿åB¿©^ð¿á*èàÃh¿éžäq%©AGNbll?ïß1s?j»b´ÏyO?H9F;:êì?BŽ^Á" Y?jÔ}qÔB?ibÕÐ܇è?ï±ß×OY?€¯*)n?R¥¾àô1Ð?X5™M)÷?3‡®
£ê?|ÒÝ~Ë6Ä?î1ËvÜp?–W P¶?˜¿þY˜Ä?Œ€¤à? ƒIµl¡?Œ¸"nÏ?ï€ð_¯Y?‡f:jď?Eٌ·	§Ï?H™¥†C?Ž«£?‡²êá3FGL J2135.3-5008@u·©³únÀG1Kÿ²Ó'À9&*·c®üÀ;ti;'§?å¦Qs˜±›@/Á™gð@Â7r@º¿â]Pì4Nſ磷쯯õ¿æ
fyG¿î97²ÚïaAGNfsrq?ïZ
8ª¸?'ƒ}Û\ì?z¨óš¯¬?x~í/Žíp?Œ(Þä}ÄÌ?‡d—Ûp?íj÷‹çÏK?©ÊJsÝÜ?"u˜[o=?'Hã™`'Õ?¯ÎLuUSÇ?¥ÅÉҖ7š?íè"ÒúøP?Ãغ>?¡Hœ•Ùä?'ñ.xÙÏ? lŠ3º¡+?')ŒÊ?èˆÅڇžê?­Èmw"?©Ç
¬?˜=™'€T?Çk%T›ÙW?¬[è¿À€(3FGL J2139.4-4235@vdڀIf{ÀH)οìºÀ8àÇU"‡À:ýÂÅ+?öùŠ¨ex@ðÀêÁTt?þ.` ©®:¿ÚÚ$¿à‰ñ]]%¿âª-qI¼¿å¹·©AGNbll?ïæg
E²Ú?f"bvðó?0@åîZº?2ëäs×'H?gÙÏ[Z?eVœ"Ä¥?ï²%hS‹È?Y™Õ?R(4hñ>J?XBŽx͘U?1Ÿ]þæŠ?€Ú—çÜK?í«XË0¿? ®æñÙpC?šƒ³tÉÒù?'}UžS†$?¨™'™J?š¯wu‰DU?îo:«ÇHÕ?¡¤…î?[<?`aj÷‹§Ó?c؅¾›p?¨>"¸E?¡m@LÌÐ3FGL J2140.0+4715@W(üà%o%À-J?¿2°À8~&vŒNWÀ;9ÕÓ܋‡@ÆèVÁ@
b)Üó5—?÷òˆæüy?ƒMc¤ÙØh¿ßæ碈x¿éÀ9ÖæV6¿ïÿߓpW"PSRPSR?TÂWUî=?Y}ðۛ¯Î?ê¤.aœ?É`o‹È(?Ç»ê™]·?ÉT)ô¶ú]?¿q)?6-¡E­o‰?í°G~ãó?¯ÕæíÞ;?²wÝçÁÜ?¯Ñ2¶¸ÿ"?š6&•ÍO?àTæQͶ?ëïÂ/×?¨2µÕÿ·Ž?¼ZøI
õ?¦ ]f£v?]ãlºÐ³€?WGn¤O›k?ïE.Ã!5?º«G
Z‰?•{ðÐ,T'?DLKÌ3FGL J2141.6-6412@t‰¢ß"xîÀE!'	±À8úÙ*© öÀ;¦þÍÐØË?ñ€=û8E@"ž­Õ'@ö?[4¯¿âuöÉk¿ço7HŸ3À¿ç>‹Q¾tÖ¿ïûdÒÁAGNbcu?ïçX¸¼0n?bÒ#‡?Oú•ŽþÉ?PðK[
?`¨Ã^kÑ~?_#Ãóª<«?ï¥þwŽîN?"±ºö˜¼?W°W2pn?dC
Ä?ƒŠW5öi2?Âr{n‹•?îŽzÔ.¦?'˜ízŒ?™.·@Nõ?ˆîÍ]n^
?•$vÂê݀?‡'\	?ï­vÍeáÅ?"œ'ѶŒ-?Qe£Ø?V%¦*¶
Ù?'u¬eÈ?ƒ¸­Ït¬[3FGL J2141.7-3734@|XüŸ£ÀH…ÅŸ±áÀ9º;Ú¡¡¦À;ÂÊ榓¿Ó$šß>êL@ÿ<ú\R@»e€À¿á·b¾w¿í$FŐk¿Øm<7­…#¿çƒÔ¤˜·XAGNfsrq?ïùÐ{¸Ì?[W†óÒ&w>óŒ\%iR>ü©ƒcª}ô?H!®;¤®–?[Â5tŒ?ï·ùÑe^?~·:Òn¶V?M¯ëÆv?S"cÚ¨¦?€(€È·ì!?|Eù¸ª€†?îÞ9çBÛ?'Ûzoû!À?tÇ°oe‹—?fU«líl?Ÿðç>Aƒ?'°:äv¥?ïNPV"?";$ˆÖº
?1^#»Mƒ?YtY†Ú?Œzï¢ä^?"*×ȗ%3FGL J2142.2-2546@7œà`'ˆÀGòˆÀ-'À:õÊdÀ;ÎþV²"<?âþŒ2'ð_@ªÅ[>j@ىÆã¿àÙ24Z¦¿áø'ÕE¿â@ª½áÕü¿ïþ½FSþAGNbcu?ï"ųɂS?‰û§[˜ê'?{NŸ÷L4?¸þˆmŠ'?zΆ$!Š†?|ë¡Ñ¹?íÕ»ËM;u?©†ÅÙ:ð¢?ŒB»'T?,Sa˜¯9?«A2œh¤?¥¹³K´ù?ì¼ðj÷ò>?£›ÂØ7…?°<ҖKJÇ?œã{…É$Í?£·T#êFœ?"M¹«¢Ç?쳘9ùdµ?¢BòKíúG?Ÿw€l"?«¨À"Á€?²œ P¶ö?žÞI±IÚ3FGL J2143.1-3928@´j¿f‡ÉÀH¡à f§ÕÀ9å)*›´ýÀ;¼÷üü??Ð9å©èqC@¾9Èxª6@•p@"Õg¿ãù/±¾¿ãSßÁy»¿ã_Ø{4\\¿Ê´ûÀ¾2AGNbll?ïÚé®?v¸Å®x?C@²tu?n·¯i§t?p( õ¡0Q?qU5ZÜ?ﯛÇÑG;?ƒiZ—?NÃI€'v—?SI…wü*?',Ùs¥;?']_`áÏ?ï@ðÁ4zE?…¨ÖŸDÿ?|iu¼Éß?t€ÆC™/?ÇŠj>vž?&ìaiãy?ïW€¿àZ?‹L{a:R¬?;؀¡aK#?F &Þ'á??" œe~ov?‹îºôøõ3FGL J2143.5+1744@R~_ìÏ¢À:›?Œ
À7ykˆWÀ;™À0X?õ'–‹SH@TI,į@Ò"¡!¿ã·+À^f¿çš+FC ¿è·¾-‰¿èќüê:¶AGNfsrq?ïèºàX?gò­À\g¶?`ã¤o­¡ý?e±¿,öŒÌ?I…ìß	&†?JÜ6	:E?﬩-èŒÏ?'ôzg||ö?\´H(Ýál?bòË,êã??+€ÁJ?€"U}Š*,?î¿3ïú?"öñ'N?–Ô&;ƀ?†Ì(LÞõ?˜N5Îâم?ŒNþ:Ÿæ"?ïì….š?(ê]Šf?^=þ§+q?dÈ+	ý&?š>ž$èz'?)¹8`n3FGL J2144.2+3132@T¥µà!=gÀ0Kæÿ}úÀ9©°â‹zóÀ;¡­SŠÁ?³ð˜-›µ!@A]Û}i¸@å¾@Q¿æT-';¿Z¿èL®ITè¿àvÒ&î_¿ØýNʾUAGNbcu?ï"#E¼^?'=8\Zu?Vî)»-Y?Z–}ð¥?Œn‹Èƒ?'+¦[\?ï|
J´a?"j®Ž?i¬K€ÓsZ?qÕùø™ì?Š'Z{Þ
Í?ŽbJ™>?îwþ%;±?"¹äRÒ|Ã?ˆç"ü·?v™ñJmåá?¢UúÞ§}ù?'
nòû?î½_™ñý?"
áp?Sçm2V"?Z@‡÷ý•–?£ŠÔ|Î+¥?'¯EáùÜ3FGL J2144.9-3356@&ó7z>ŠÀHÍ«ÿÍ«À8÷¨§b°À;¸£J"?ça{aŽÿü@f2R7°@\–Þ²}¿Ú‹¨-¡¿åŒv¢¾¿å•GÄø¿è}
xAGNfsrq?ïóáûñµ?RÊhÙÃöá?<Ý3•"´?7w¤EÐÈl?RÀD»76¬?PæÙ:sŠ?ïÀ¸Lƒ½º?~
ÃV€]&?J*{8V)?QY\S6G?|^ŠW]?{ûd¹xýs?Wz‹`?Ž|zRh±?›ÎÿB'´?€Æ hÛ?™=
'
RÒ?…'âgæ˜?ïÍñ²ñ_œ?{Zƒlšÿ?'ÛFƒ¢I?0=öHñB‹?xHLS7U–?zÙ?!+ø3FGL J2145.7+0717@OÄ"}À@µt@C¼îÀ9¢ÓßÅpÀ;‹N[­¥ÀÀ'(–ÍŒ@—f´=@@m`€žK¿êö¼»:[Ï¿æõ;4A¿å}©gå9¿Ì#â.‰AGNbll?ïÝc¾Ö^/?mwÔ}Ïå–?FPY·9¡U?GfC«É{?m*»ÓiÄ?k™Æ€µv®?ïŕof$?zº?"ï?H§öéjy?Qâc}Oöø?z I|°È×?wè­
vc?íûZº?˜Ä\Œýµ¹?'d.Q'?€³";z¾Ï?§D-×ûZ?"}EÊ¡24?ï¿Ý–µñ~?yoàõØ[>Ûät:/Z>ï@6‹þÁ?€Ãü`%?ymô¢…w­3FGL J2146.6-1344@DT—b%ÀF|ŸïôðÀ9sñidHÀ;t•?ñþIQW¶u@þ¹+ZKÑ?ú}ÿµ,r?ï°'D"?ߦW{¯\¿ØÒùmzèæ¿ÒýGbƒò'AGNbll?.z	í?ª5Ÿÿ«Ÿ?"Žåñ¿?"'lyg?¡Ö|´¥äÄ?¨›ÈɞV›?îûÈ´õ?Ÿêa",0?y¥@–m_¨?¾bð|[F?š66ÃàɁ?šD"v	Î?è¸ã'ª?²K
1°TN?¶56¥Š¢ë?¡çéž5?Â1 žWä?®DM[9?æaò´c?À" Ӄ¶"?¶€@JÖ³^?²ÓØ$'}/?Ë8	JP?¿—ĺHŠú3FGL J2146.7-1527@C:\?›÷BÀFØäÀ™,À9åVI¸±À;µ5õ…R»?×¹¬%¯´[@Éª@«À#Ç¿ßíÔߟ¿è¾Zâ,c¿êaJ"wbQ¿ÌO¿iüŒÈAGNfsrq?ïîÀ¹ËÛò?\:9sÕ·"??,Æsݝ?Azhµ_?Z³ZËPµ{?XQZÕÊ3?ï»+Hò?|)š‡D‹ó?J¼W½ÛnÅ?Rää¯^	«?Ðø¼™9?yôTcïù6?îûHØL ?‡àú‰.å'?†¯þ·¸Ï?zøU¡ZO[?•>åšñ¢?€Ðë÷†4?ïO°¢™º?ÝÛm?HÚÔZ¯G?Q³ ãÊ?•C'È܋x?Áèqò.3FGL J2147.2+0929@PsìZþÀ@#%¿­)™À8·	)7À;?ä^¹É»?ö‡¢äß@±·Å(¾@µƒ.ž#¿áh¯¶ˆà¿è‹A".¯¿èn~K=Ë¿é}ÆTb­ÊAGNFSRQ?ïò×rý?R13hQö·?OÅY_Æ?Mš¨£Ý?DÝ3rQÍ?@ù騚;?ᅦtÂ?{è\½‹Ì?QYE×°ñ«?[œDgU›?{åô‰²ÃÆ?w"ÙQ¼?îÎ%(?'PÖ÷'¿³? v˜?ƒÑ8;ž?–±pæ?‰˜dDú?ïÁèh?LÚ?"7W?2µ\9?AÈÀTå?}àv…úB?ƒú¡Á}s"3FGL J2147.3-7536@s¼®_ú;›ÀBD-ó»NÀ7[ðEwÙUÀ;/†è¼í\?ø˜‡Ô3s@Û6"Q@rÑÊãh›¿ã†ž%€©D¿æ销w
¿èÝz!·¾¿é@«}‹ŠÒAGNFSRQ?ïèP~5ß´?aXaý[vº?Zìv‹õ?[®ýýìÆÀ?UH´£A?PHRkÉ?ïÆ~¿j|¥?xj®þ?Hœw1g?TîòôYÆÌ?y­ˆ2Ç¥?u|"\9
?îíØYŒ4?'fïjSé3?ŽŽR·?¬¹?†Z#¿l?'ýËrÙ¦G?‡Š†ø —F?ïø
t' ?]°"y<*J>ã¯
"'>ú¿švíÛ?O{qÁ-' ?]¬j:kªl3FGL J2149.6+1915@Rœz?̞ªÀ:
Û L¦¢À9VÆu'ÊÀ;sCWm¥?c©te%_@Sz'î.Ç@Œ' ;¿å
ª
7ԋ¿çE¹*-¦¿ç›@'{Ï¿ïÿîpǤ€AGNbcu?ïó+"Ì´x?c*^ÁP!5?,zˆê^Y†?8múï˜Á?ViIKC°?`é»]Tií?ï£á»íŽ©?Š‰ÊšÙA?_1>yÏð?bèWšXë?ƒ!i5br÷?ˆéq.ù?îër;Î÷©?Ža+W4?'%SšI?…\hů¶?'r`Íp¿?"9i4öð?ïð×È?I^Þs?aÊW:íÃ?c›1SX…?œÚÃý©A?[+Xå‡3FGL J2149.7+0323@NFâ?û˜'ÀBQ,_Ú[+À9˜ÛÈRéÀ;©¼®q—ó¿Ö s8ז@ÖJHùn@4ƒPþ¿ä{Ÿá1]Æ¿Þsñƒ)Y"¿álš¨7l(¿è|/՟sAGNbll?ï¥Hºßú1?‹C¯	ƒuƒ?QÙâÉé×?V‡Û:®s¦?"r"îߖ?‰j·w4µ[?ï}ˆé½Ü?‰êEª–›Š?`Yô÷ú'?bdc¹)U?Œ‡HR½¨J?‡È¿Ìòûã?îóyVåþò?Ž±(­Þ}?ˆ©w°ÞáA?€W7ÏU#?•<JбJ?"Æ|"}¶ƒ?îàCXkŸ?Ž¢ÈúX?[;Wªk"?Y!¬	Oj?¡#žâ¡?-iè´3FGL J2150.2-1411@DMþ_ìÏ¢ÀFú?Ï"èÀ9ÉΠ£¢À;‡ìZ0Íþ¿ó9‰®¿ñr@Â}'Þ[?ýB"!=ƒ¿ãYß­5i¿âÂ:Ƌ¦M¿ÌZMN¿ð¿â‹t™É®úAGNbll?ïùåO¦²I?Fv1×-†>üQ–RSñ$>ÿYNo¸}?Gˆ4²¤;@?F6‰93Td?ïÂÛó‡Oª?{Z¿M¦?G¬áGȃ?Qm «ƒ/¯?{œj_'?y9Þ?ïaP} õJ?xµÖÜäØ?uŒ#ê˜?i>DMÌ?0·÷?}—ßÆô98?ïŠxð5|Ã?ƒrÒKXæ>òwPg"U?<)
¶Ÿ?Xˆrx›b?ƒoPÙÖº3FGL J2151.6-2744@5PÆ3¡îÀI*èà(Ê$À:'e"'ÒÀ;Ë5™?Ç?Û/ú?\ó\@/‡­@Z€a¿˜"³ƒ´o¿êÂ#ë0¿é­"b€~¿äÔ%¥<KFAGNfsrq?ïÐ=[^¼?vëk1+xí?iôy©Ø?oÆQ["Â?f1°'Èj%?mÀ`ì½DÇ?ï[²`jA?"r´¬žŽó?g¦Î8‰†?rÁeý¿²É?'"Ú+¦»«?'w(Ý2žÌ?îЋ?ø?–ŒëPP/@?™óÅà £›?ÐîT»M?¢é6û®™?Œi^FÀTG?쨕ÓJÄ!?©MãS>ƒ?Š"£9ÁÞ(?"v?-´?·h¼þq£:?¨ éۛ"83FGL J2151.8-3025@1!Ef­ÀI`Æ báwÀ8>ŸªÀ;cá6]E?üó¥&@"¬Âc¿@	Eç#»¿çŽ:¼z«S¿íÒ_³Ä¾¿ï+¢^Ô¿ïç®ÀGXYAGNfsrq?ïðDvº¹?oîZÈ=ç?Scª]Æè?f'æ¢Gõ'?HïšYˆœ?`ÝSïòß½?ï¹Æ¦H"q?'Þ'Q–y?V°ž]åD?u­ÀOñM_?}p…DtΞ?|xy!¢X?ëÂfV×W?¬Ñ—L3È?·Áó5µ»Ê?©ù‡gdÙ?¤U´'#Òï?›<ü"	ž?ïfFHte¡?™jk]"ïâ?kfŽ,:!?wú	G5?"ÊWØB?—.Þò')3FGL J2152.4+1735@RidÜY2À;±< BÀ:"曪ëÑÀ;Ï"‰G<?Óuö
°9;@LxiOò@i3ˆf¿ìn'yÂc½¿Ò¨-}‰¿×'e/뼿çÎM¸<yAGNbll?ïŽ*³Üc?²"ñ/pnç?Hߍ?PÕ狶µ?Šó}"É?² v•ú8Ž?ìÊôxú´N?µŸŸà?¡râȪŸ7?¡ÖÄÁ4A?°îêÓÕ
ú?°d‹+~g?î¼ILdðá?Y6¡m Ä?Š¥^tYzu?~UôžïÎa?›$'95&©?†û¸yp
ù?ëæ‰FŒI©?©*¨¨>x=?ž¢CóKÕS?–6&‹ªÿ?¹#$Îʽk?¦Ÿ'c¢‡_3FGL J2152.9-0045@Lw©Àª€ÀCÞÆ_ËA²À:I´+'À;ªÕ¥¹cÀdfÇ_Oœ@=½O?ÿ)"_è¿ê¿«4²ËU¿¯anAž}¿èòÖ¹¾0?Ñ]²eöÝuAGNbll?ïòä¤T`g?Z‹[Nâyt?Fƒß0úî?T]c¦0‹?MêaÏMbá?Ké6ÕÁ_?ïŦDcÆÈ?z"폍n?IݘfPðž?VêQ'Z'Œ?yñ*ÁR}>?wj1×ŧ?îÅ'ÙÙ:?ÈÔÿñ*±?'¨È^†ç?^È'l^?¦ÜfQé?…¯§ Ä>s?ïÔ·êÀœ?zÉÔ½Ý7Ó>çê@ü©Ãø?\@l"¼H?uí®ê!]"?zÊPhW·3FGL J2154.0-1137@F>T2TçÀFÔÓßæ…À9:̎¹kÇÀ;ª¬ê¯5ã?î"Uk±Ô@}Ísí@é(€&ÖÙ¿â@4XLGV¿èO'²v¿çƒÉü¿ïÿíÊ"EAGNfsrq?ïîªv—ª¨?`X…rrW?;.¼®|5Æ??åÉö.b…?[ßc¥£õ?]:ã‹ùoÔ?ï-wMðY?"["Ì°¿?pf§<b¾š?wÆóŠêõÍ?–7l‰E?ì¯N"O?î|÷§=†?'Œ%»BÞì?˜ê¸#Ø?‡Ӕ…5Z?˜\·	`+C?ˆ='Ìs?î?'9ã?£šgÛMï?Œ}š¦úÆW?†¶Æ%`?§ü¡2£1?¢,Ò0[3FGL J2156.0+1818@Rº6ŸÏ=ÀÀ;Ê	 '²À9ôW(ÛÁÀ;š}=B€®?Ç`d×ù"C@¸]?÷î?þ `"=µ?ïüà*D«¿ãÿl(¿‰¿ÓäŒ&iv;¿ãÓ7m©"AGNbcu?ïìË®è)?ci0lê?,]ç|O)?,¯˜	ƒìÎ?al;9m-?bèÃY/?ïƒÐ¿>A?'ò›Ù{?q?d7u'CŒâ?hdúZ՜?‰þ!ëߌª?kæ<dl?ï.Äâ?‰ç{7ĵŸ?ƒ$µç"Õ?rþ]éå¸?–gâÁәõ?…ÓGB±A?í§':‡?¤%bè}«?eNÂÉ0ž[?eÑx‡²¹à?²øÞFÎ?£¹¡]ß6
3FGL J2156.9-0855@H.­@?‹0ÀF HtäÀ:t䝣êUÀ;Æ£iüóÜ?ÁÜ#¾r@M¯gQî?þm'Ԇª?ïñ½øÒì?ë£`Æ>F¿è'ßSª¿°¶¤cC"AGNbll?﹏DÏÁb?'sZ=?\¢@¼¬Ü?`¨ñàúÒð?|Íhôž?
¼D8ƒ?c(õ+?'7÷£²©C?aHæw_ó?'gÌ$4¹?…€-µ$Ý?ˆW³¨`4'?î
(RœÄï?—9⊜À?›¹ÐÌ)ù?ê4;i5©?¡P'p-?‹ã®Ë;?î†ÅÃ0Û?©'"ŸD?˜b(=•Äî?¥"·ÖbÚ
?–Å\f_¨?šõ4àm3FGL J2157.5+3126@U0m_êKcÀ2=²?'ÌÎÀ7ž1œZ>:À:ôŸÅ,Å[?ýºOq­A@¬:ŸŽ%G@¢ø{§@¿Ý9: Íâ¿ã–δ¿ û¿æ_8`ÞUû¿ê¡¯`¼iŽAGNfsrq?ïkõuwû?–gÔ)œñT?…±á
ӊ?ÊÉùÕ¹6?€1Á"-¢?†ö­.¢"à?ï¾TT…Šh?ƒ¬É~?X ç,P+§?`áÜ£u— ?z͛ò&ÁM?€½YRð!O?çqc×cv?²Þ†h\â?Å$'j¢?®ÅæؚÛÔ?º,«"	?¤ws¶«›?ïÌçK´§Í?''ÂTô‡?1Ë¡âbm?F±»æ_Ì?xo ŠÃ)?õO¦›\3FGL J2158.0-1501@DOs€*\ËÀH ö½À9+äŠYÀ;"C/Ш¿óòúX¡,@^‰x9M@'Õ`EK¿ãyGë=|¿ãàã»âÕß¿åu(ÐGšb¿Ûª{4åÍAGNfsrq?ïðNSï?`ÖÜ@F;d?3šÎ	êq?5vÞë;Ó?Z¿ÅÕª=?_N4Q2º?ïÁš#é?£îs^6?Fòíúå~Û?T^VПä?|Y™s'[¤?€™hÊ)=V?îۉ‰[ãŠ?Ž'à=A}?‡,óx»?{,}÷èª&?™¸ZÇ~µ?‡³8¢ÔÏ?ï×'FZ?qfë=Û©Ü>îu¡<1?Vׁå»?tm«9Œ5>?q`‹çùjn3FGL J2158.8-3013@1º¾`"‡ÀJã?ÕØåÀ60Õñ8¼àÀ9Ïù‰Ä:?ðÚº1¦k@µŽM5<ù?ûCÁñQ'm¿Ò
¡ÞPr¿Ý[4Z5窿ٯ ›¾7¿Ú@µwp¤ÙAGNbll?ê»øÔ"÷ ?ÃÚÅt³?Cß¼Î)^Ú?RqÁ™x?Äü<ò¥ú$?ÃÖL#hBs?ïØþ!€EJ?tz?@ÇH?Aq[ó,Š?H«"S®'W?qRÃÁ{•­?rÊ\ÂZ_þ?å~~aï?µ7ÌúÒk?›Ñz
?"o³Á"˜›?ÓEì#{P?´v8³÷÷e?îHŸƒb¼M?¦Õs˜™Î°?ø*NÉðÐ?Äe<u?«qÉ¿@ˆÒ?¦ÒgQ©ñÛ3FGL J2159.2-2841@4<ú?̞ªÀJ¼ .ßÀ:¨y0nÀ;´ÆžµbM¿áäò
¦f@Øe-VOm?ÿSßûþ"¿ê³A¥*¶&¿Ü1''©Ô¿Ò	nÕ1˜¿åG‰óD—AGNbcu?ïöl|W?Q9œ¦³ ?&Ú@†í;?05 Q¸©¥?Påã?@:?NRt–CÍ?ï³	mõ~å?È$a9Ÿ?R2Gí{ž¸?V™Ü¶.‹I?€÷["ðÓ2?|\5"@ò?ïLÒ#˜@¢?"4~Pª¾U?{¼×ÞnžT?l÷àò¬ï?Ží*¸ˆ¥?€)Kýnßí?ïOª§Õ2?…Ühv°ã?*
UÕJ°?/–G…œg´?•Ö§ßZÄn?…½¦àMCö3FGL J2159.8+1025@QFàà¨.À@ú0ߛÜjÀ:þñ´
À;µu	—Xw¿ÓK!ÄÿW@ùô+¶g0@% Jù#¿êS?V›ÜÚ¿éλžônʿȑDá[z$¿ïï{¹ðã>AGNbll?ïÚWÅí/»?…T"
Æ}?E­2Ûôw?OÝ%Ýsü?pv­é k?"ÔÐÃÖ4©?ï3µŽÌ…ª?–?Ú~öùâ?s	 Ö¹Õ?xLþQ¶Y?"ÇðÀՕ?'Â9Ë°?í~A­}(?-¯œ<
m?¡×òåXgÐ?ãm˜» ¡?¦CûÏÏŲ?•ý/àš?î%"ñb/?¡Ü6'PqÝ?bå9³p®?jóêcDz?¬€ú5·æ?¡"ƒ«ü3FGL J2200.2+2139@S'tÀ0ÝÀ:6_7üÀ:°àÝûÉÀ;Ý`ÖÚlÉÀ.Ð ¿=B@ŽdŸfã?ÿ£k_I'™¿íx[â»ã¿Ç	$6@-í¿Ø]Ÿe`'¿ÒQh3VTÝAGNbll?ïüg';¼Ÿ?;â CåI?¶ñ=•0+?IÉ·Þ?6V1Òµ´c?9y-åR?ïÆ?Ðb™k?y<¦­Ú]?QÏ…{g=?YZ
À\?xlQ-Tpª?vžlUá?ï$ÿT•èÝ?€±@S)ò?,Pá³B?oéýŽÍ[\?'×DÒ
·?yz2Þå{'?ïÝ?Àâö?k÷Ãîá<
>׀èÎ~C/>å45h±8m?qZ?T¼e¶?kòk'«T3FGL J2200.9-2412@;}"V!uÀIÓÝà‡kÀ:H%"ü|À;â½ F?¥½9…'‰Á@e›»2@¡³_¾V'¿éƒëûnÔR¿ëuÄÓ·«0¿¦õ§•
vi¿ã)åz©Ð…AGNbcu?ïùžº8Cš?Hâ·Am®>?§ó«V«Ä?ø{‡?GP©†¾Á?H1î#Ê?© sC?‡Ï¨÷M?T<÷ìF?`_´ïgë+?…50D1Ú?…²œP¦+?ï
G¯@~J?‡"¬ªº½?|õñȊ?k«ùÜæƒà?—¯Œ›©Ä?" jÃÏ*Š?ïFt¾­Ü?'Œ±es"?-Ô@Jr?;‡_õŒd?—É=©)³?'yϑL=ã3FGL J2201.7+5047@Xi"d¯À^ƒ¿èÉÀ8).‰À;5/»¯n?îkÀÀSJ@r'2Ÿºp@¶Óàg^^¿ä$`gÒTÕ¿ç6ÃÝ©­¨¿è®n4]w!¿ï3Š!oAGNfsrq?ï°ƒ@ ž?ƒbHKÏ?z+òrð¿?{oæFóÞå?k‹—ÙD?pœ—sÿÌp?îµËºe
?¸N_4í\Ï?qç¢o¦"?–/X‹?¢fPºŽ?¶Ìÿ,\L?ì_ÈR"Ô?£¯j$l?¬»¨1…Ã?˜›ÒHé>‹?­GÒ¦,ûP?™©;û8Ä?ïý.R©Îc?J~Ýåó­>ÚfÁ³?ScO«â2?6#Ò2†ã?JW
ôöÔ3FGL J2202.4-8339@s?÷LÀ?¼±v/À8}¨'j¨ëÀ;³¦‹¤?ú>ÿ'ö×@ºæ´Õ_C@"?(ßÈ'¿áðÆËÅ«¿åÁªRàˆÓ¿è¤ÃðÉðé¿ïW¶ð9üAGNfsrq?ï"3úœÿ?†¡ÿ=n6?KÚ&™8?"B>õ"p‡?sNNeCDè?s:;á7ãó?ï¢qBÃú?"]³ø\?Z³nD渁?fÍ-bty™?"
A±ò*X?sµM*JÅ?캫?Ž?¥$Øïs"?°Á8=ÊqL? ¸Â*F^â?¢Òیr<'?–Wxï`@?ï"øv:?š¢FJ48«?pUã;Uê–?€4ba×?›Wè"c3«?˜ì¹…ûµ3FGL J2202.7+4217@W&@_×,À$á'ÿùJÀ6t _ñØÀ:…nÉw-?õôò°·@0áhv@ã±jƝ¿á€…15_¼¿ä©§…âÏæ¿ãÚÓíõ³Ã¿å±ë`œßAGNBLL?îµ |ós;?¢MŠ­Sc?KÔbD¦É;?O:,ôÍwê?¤6¦§¶16?¢KI À#?ïÇY"ç?ï£óx¢?QvìÀá¦?Y-[`dŒX?wõzAÇi?{ÀBpP?êñeȦÚ?­ƒ+z
^ê?›Þ'%-ha?N'ñy?À¾™\7·‰?©ÅªÏ,fü?ïòë#Þ?hrôv»ã>â¦tÛÆ-?¯µ>Õ?Z~Ð
¹†?hnK»öÞ3FGL J2203.4+1725@Rëà
ò1À=£GàiaÃÀ7»Šˆ"ž`À;Šrµ)B?ñååóö@ڜ#·•-@QâZþ~K¿ßð0$ò¿ãðk"LD@¿æ!ÓÉã…ÿãSù¼;|zAGNfsrq?ïêöU3YÂ?fRKKV*?9NPy!¨?9«éó»ò
?aßàÈ·?eþtxÀ?ᅨÆb4?zþçâ»-?QÆÙ÷Ÿ Z?XŠÏ¶ø©?{ÈfPþ.¯?xûi–•Ó?î,ef&á?›s¼î¶[¦?"µü™Çf?ˆ¶À-òÏ?£cË]®5?•
D¬©È?ïºNPŽÃË?ƒð©!£? Ú~ÅÛ?3Þt$O?)ä8ÎH?ƒâÃËBœ×3FGL J2203.7+3143@U¸¿ÏŽHÀ2ރàÊ°"À9 Qðœ5À;Pf͔ÀŸPõ-¿@'=Ì¿5à@†‡_ZX'¿çšøO:c¿éWÝ÷cñŽ¿ïÿÛ¾"_T?ÚW·€¤AGNfsrq?ïúÙVÛª?B]¸_cìŠ?3‹èf=2¿?2ËKm×ý?5©g2å'5?:S&¶F™?ïÆ'>kåØ?üOâ=-d?U-1¯¢Ïæ?lš"ëÍA€?w¡^$_Ý?z¾`àc8t?îÞÏØlê?ÒQg^?"Ò.®E`?{$°¨@\ý?š›ç;@&?‰+
ªÓ¬í?ïë Š@Œ?lOk>¬agjJ1½>ÖÄ8]㪶?dݯ©qÎT?lNMC¨Öa3FGL J2204.4+0439@P.lŸÐë?ÀCSçÖyõÀ9îévQÀ;Ãr°÷"0¿Âîªzüö@^Óª¬±@þ=ß^ŸÉ?Ùlé™BS¿ÚB»ú "R¿ëM豍^Ö?²uµ"(üAGNbll?ïÃu‰Ûµ¢?~²p–t"?p"3Aœ³L?v†¼AºV?kb¡ø[?l€36@?ᅤlǦ¸?yÙh>±«?KÙû¦ÀÁ?Q¼EÒÑd?|Â
'TŒ ?w¿;&á‹`?îwÌÌT?˜ºn&å¶?Ÿëa£Ê''?'ed¹bBR?œb¯b›óg?‰Íý²š?ïšéÊ]?Ž#"%¥Þò?BXW¢Ó—?NCÇà¸ê?ŽóõK`/1?Ž	þ~™3FGL J2206.9-0031@Mú¼ßï¿@ÀE6ö`D
vÀ9¢T™µHLÀ;ªf̽³T?ÐXá"-nÎ@Ûhêz1Ê@üâo\¿×âK€K¿âæ‹Ôx×q¿ãï/Z¶"â¿è~ %ò$mAGNbll?ï²äcڒ?üŒÈ´ïê?csènkão?dU
Æ­î?|ÓËÜŐ?{¥¾Mø™Ã?ï5TºÅ?'#°,ÎbP?l
›ä•o"?kebX_Z?•Óµ3‹Ùp?‹sø73?îuEØwZÒ?'iårˆŠ9?"'4?…ýêºëžÑ?œÆ&Úúpû?ˆ[;/ѱZ?íŒâ$5R?Ÿ¦8õP¯—?† S|?t>¬#:ô°?± "Ù®¼?žÇÔèzÅ3FGL J2207.8-5345@u>…ߨq¤ÀHøm¾iÀ9ôÛö5À;̪â—9m¿÷?´öÂ?@\Ý%µ@ªå_ë¢ü¿ç~"ƒ
¿åCîÛ{¢t¿éjÄzÔç`úû©ëAGNfsrq?ïûÊÈ£3å?A20?ážj?#fvaêiâ?$}°¡èä¿?7öµk¥?<Ù®'QÅ?ïÌωªn•?x§fì¿?F5ûm?Ã7?P±ƒbJ ¬?vÑ{½ ¼Ù?vù¤#é?ï%~ìÜ?…[~^›Â?žÙ×Wÿ?ro÷Xqð=?"h‡ì©DÖ?ÍZ*ƒW?ïð=mI?cd¯ÆÎ×¹>ì£
½ý?	>g<'?_L…äÿô¤?c?Pø¹3FGL J2212.0+2355@TŽH¿÷Ò4À:©?ÿÊPÀ9}K…9À;†ûß	?ÕKêßâ@,þ¯çÝ@²Ô (>Ž¿àÓý鮿☐MH:à¿ã«Àsß1¿ãr`†Â@FAGNfsrq?ï%•åP?N¸†i'?oípÉ­?p},-R®ƒ?—O®Ⱦ?›­Ê˜u@?îúi]#Æ?¡ÛÈ&‹?~йc?€"q@w>?™5Þέ.;?ŸÓO9pb?ìøg ÄÀç?¢W2•S?¡kF…Í?6‰¾G‡_?¯Gó.ÙÆ?š¦"è?줬¬ˆBº?¥
aø\?‡Ò."a‡V?ƒXҗ}Û?·àTÉ1¹F?¤X¿Fóh3FGL J2212.3-7039@sôî²ÑÀD‡"€,á
À:${À;´»¶úÓp?ìû–dìúÑ@9`؇ëò@}\¬~¿ç£ÿ¦5UÅ¿è^VÚN·ë¿ìJ¦b2'½¿ÙaÿrAGNbcu?ï–ÿ9Á'?…뜻fg?w¥¡{p?{šqň?}N»K?€9XáÚ?í·«`‡Gù?ºfª kµ
?•Òâ¦sœz?§ï¼ä‡?©›Ø¤Q²E?°WåÚ?ìÀé²Ëñ?£
àrdm$?§«UpúÒß?"íìœiïJ?³,Mùì7?›nÿmS?çОÁ‡Z?ÀúÎ?1l?º"úääA?¼t@%‰¨?Æß³‡‡pu?¸)z˜¿w@3FGL J2212.6+2801@UK2-LiÀ6û.Àë­À9ðÑ@±¡À;Qøñ?ÞwՋڋŸ@
z£?	Ö?ü¥ôÞä§_?îñÇ53=š¿Û⦖ŠÏ¿Ïáì"b½¿Òې
m•žAGNbcu?ï×Ǻf?Šg4ܺ¨?dôé4	_'?ilq©5?†ŒÓÄd$?‡•Lz¬u?ïm<"Œ]ë?—&ç%?h?míú·üÅ??s!Jé;NÂ?5\.éSª?"6ÆKýÊ6?îWjÉ#À?'í¬œæ<Ç?'µžä²?€·di
½?¡zx¦îQ"?‰ÓfæñVô?ìk˜ÇªþÇ?«h=ò.úÄ?x9"îßë¶?€~›{Xex?» sº?ªãR&íÚ¯3FGL J2213.1-2532@:UC_Ñ ïÀKQìàh‹À9™TpšÀ;Ñ&çËUÔ?¼ŸáA+¢@íÓW«c@`e@ ¬s¿ãŠn'!¿åÌ3[t¿æ¬K¹xz¿ïÿõ•æ(5AGNfsrq?ïפ;#Q?ž	î¥-ý
?Dr¬IÖP?Oɐ«IvÏ?q¬TìC?ü{TùMœ?îÚóVÈÞm?¯}çñ@H?|](ï‰Ñˆ?~#1áæ_?ŠJë½ð?™ÿ£6òQ?î•d§¹O¾?"(ݏ½pý?"RÃlÈâ?‡x_g€zö?™§œÎ?L?Œé}ê?튇ã ÀG?¢úF‹ƒ"?'$àã"?ŽÉÓ֍?®E}Ý扼? "ZÄ_+ã3FGL J2213.6-4755@uÀAà?pXÀJ"õƒ¥À:Ú'ˆ-aÀ;òABÀnð?dz¼G:ôj@ÇÉÅÜB·?þ;þÝÁ¿èeêG(ó¿c>"0hê¿äxiRÿ×;¿Å1݌|iAGNbcu?ïÒ{(˄?u#îªå?P²÷g·?S£µˆ2?r•ú-À]]?rŜœ"?ï'ݾžT¤?Œ""—×;ò?Z¸£	«?gßå…z?‡ñ~·vuá?ˆØ"W%ƒ:?î°Þ-*w?Œ9y•To?Œ+ü9œç?|5u£›/‹?›Ù$\"B—?"Š6"¹úÛ?ïƒAâK¼?l{­1‹c?mùÞ^uPD?tÅr>²¡N?˜P[÷çÞ¢?ö³mnnS3FGL J2214.6+3000@U¶¦ßÓ9ÎÀ5ª¢_:øúÀ8"kp'b"À;k/¬•õ @1Tc¯}@¦ÃMÈ
?ûÑE'ñ6¿œ³š~V·¿Û˜Û¥úó¿äºˆ‰&¿îwe_*\öPSRPSR?Y¥P™dáJ?dþ§û£§r?ïÝ©÷Eçi?"¦m÷ôâ?eƒ`mf%â?z×Wfáj?]ý!Ž˜?ht)ö˜ðî?îyjü!{?¦'vÌ|½?§yg1òӛ?¥Œґ"o?'í­RD>Z?ˆ<5‰²`?ít—JÆҁ?œïÏ5'm?¯¿´ªp¸³?—ìrU¼™?x ÙB±x?pÁžÕ¥Rt?ï!ì0
?'j«Ø«i?•Úz7©RŸ?Ž>%,ù3FGL J2215.6+5134@X÷ÏÀ1³×À¹vÁçAÀ9žý†¨üÀ;WÊÆb?þ¥y+û¶@)"×ëŽÚ?üÕJœ?Ưåi'I¿Ûön+¸ý¿ä\z&.4h¿îÜ)µþLPSRPSR?kLÂA6?gÔìÝ9tà?ïsãƒ^äL?'1
[ÙÓ?Œ4æ\†?ŽÐ‡1—Ë?b
o÷n	?pƒêcÈÑ¡?èät9¡áÏ?¶2Ñ ´Ç?Ì&[@›?­µå'*õ?œ¤ÎŒÒԖ?Ž-õù<³?ì‡fÎZì?¡î›èß:1?´›•éúÃ{?[H'éy?µ@~º#>?žéÉøøMë?êÖt$êÙ{?ªgLÿž¸?´OYïä?¥t\……|)3FGL J2217.0+2421@Tâ5`4>À:u§€)ÚÀ9;ٕ2+ÌÀ;‹õ'¾´?ä'ú¾z@'/ó7Ŕ@¸Š`¿Z¿áœ坠‡¿äÔ]eòßA¿ãªª=€¿¿àãšæîAGNbll?êÑ_ò@ê?Á~ÌLs?˜ûo]kÞÏ?žì?¨Î§?Ä­L"‰€}?À‹˜ä">?çä
)úàM?ˑQ¿w$d?¼cHßÛY$?À[ÞJÂ?Â>&è&Ò8?ÁOÒCè¿+?ê§~»
‡C?ªí¤¯P\?ªfâxè:?•5¸uyŸÑ?½˜ë}Ë?¥ãÅ)|åZ?â&¿¤>q?»-Í0ºq¼?¾ØƒnS?µÓ7ê¡'?Óüߥ"»w?¸øaÞ¶Ì3FGL J2219.2+1806@SÜÝ?á—_À? íàBËWÀ9ö-Å5(×À;Ålґ2¿åŸLv{1z@Pš¢-@	qŸŒ¨¿áöͅô ¿è^ß®ü­:¿æˆ#Ó¢\"¿å¶"ÞAGNfsrq?ïÂ1Ú+…Q?"Ð܎çĕ?DԑŠ-¸ù?P¡AÊë+=?|L€¸÷ d?"/)·gÄ+?ï°²êõ4ú?o&Ò¦B^?R½N´?Uêpâ<Gª?{¢øÜ>o?|öM9;Œk?,aS?…÷ÎjW¤6?~W‰'Pü?m†¦pQR?•U쓓A ?'7ªã–ð?ïsˆWáž4?ƒukæȱ§?6‰D&2)?6äõ{èú?'4Ï» °?ƒHS%ûÁˆ3FGL J2220.3+2812@U°p@üÀ7ۚ?±Æ·À:†Tò ›ìÀ;Ëö³P$¿ê!È!õѱ@
SÙñÎd?ýU'Á(¿éð…ӿ݆³Äí°¿ÕjäJúm¿Ë²¹¹­AGNbcu?ïõ'6Ž#+?V70öÓ`??­+û[ì?Ò睒;?SÖÀ$åI?UĐO)͐?ï¾_£Š†?{çÆÇ
¥E?T¨	`'|?XGuîXØ.?{¦+âÑ<H?yŠL¼>?ï'×î?ïXüiÖ\?€
Ǭõó?j/쓰¼Ú?'û+×jwU?|Úþ£´U?ï¨c^*ó?{J¸¾ë7ã?͆˜'ó?&D75øJ?…ËZï2§X?{@Ò¬t)B3FGL J2221.6-5225@uE¸Ÿƒ¾fÀJ2ûÿÀ? À9`^SrmÜÀ;Ó~—µ"¿ü˜V¶E ñ@+óSIS0?þÒ^ß´[¿à+hjìÅ¿àŸÜo4É¿¿Ú«`êG¿ÜšÖœžAGNbll?ï"KPæ[?…ŒŽ²ƒb"?CÕŒG?@W€=CJ ?‰»Óçt?…"5ȸͮ?ï¾¾
:¥?~¶ÛUÇÎ?M¯Â7]qœ?Vƒ×"—#ò?|ëÁϹ?{H¶®°Ý?íÊÜ°¹h˜?›8âøh?•+G[¨Ó?"®`¨
ßN?¨¼ªP»¢"?•*…ˆØ·Ó?ï1ÇÔˀ?'ÍŠC#v?zíМg?ädGMÜ?™ÑIŽâ'£?'Éow‰Ÿ3FGL J2222.3-3500@#Lßàû®ÀL¨ñß«Ì¢À:ƒ¸:lãÀ<-*ÛuÝ¿ê‡Z'÷@Þ¬FD‡ï@ùã_`bÁ¿ãU¬žcË¿ßÕÖқT¿èÜÆè1W;¿ÖDf'§ûAGNfsrq?ïõ' @¬?q3CdgÌ?KajB½d4?lÖބ³z?@'<?ì‰?M҄ RÛv?ïÒ6‰¬H?w4"xHt?Bñµ»&'t?M †G¶J¡?t†"rw3ü?uŠ·=t?îü'Ñzy?Œ(fì}?‹[.9Û\?ƒ­æu±õ?'ïX9"ï‹?Ú–VÕø÷?ïôMšårB?V)ÎƾÊ>ÞB"WLz>èZ¬ÐC@?WF½òù'E?Vžû"߃3FGL J2224.6-1122@I$­€k`ÀJì@/šøÀ9öÌP¦
ÁÀ;¾ðù²¿ÿ9H*¼@
±Q؏Ε@'ªo÷µ¿æ‰¡Ñv¿è³ifƒw¿Ò0ыšÊ¾¿ïùÓKþ'AGNbll?íýYË&"?²Ú5Úªpû?kL»®hß?vwË/H?®u¢ÓB°6?²<@aúg?ï…;¡5~?"ì1€Mp?`¶p£\Ð?tõQ¾}ŠO?Š¯j Éɓ?'Š›£nÑü?ì\ºíGƒ?¡"uð…?§RÀr°Ñ?'ñ#LHUc?±v' Ük…?›h8T›?îÔd&o
?Ÿ\æ,?/¯—c´ú?C˜>-:}?¢ J&5úv?Ÿ‹æäO]3FGL J2225.8+6045@Z"O~ÃT~@wàmòÀ9܋Ëz½6À:ò
kùM^¿òÎ?`"Â@ŸÓŸÏ¾š?ÿ&´Nߌ?éÅŠ†`¿í 4é옿ҸŠ©³¿Ãê­ÈГ×OTHERspp?í}xÓå?º\c:ç–v?@,͕Zô?AV‹M*cV?³ó*ž="÷?ºVøâ‹?èfCÞy?ÓtÏh>O‹?ˆ: çžý?›yC!ï?ÎÅÔv¥N?Òá¦âË?é¹ò¢U?±€ÉÇv®´?¥s̆?†'Rk]Ï?þԊoµ†?°3Õ,
y?íçœvmÝi?ª/h[9¨y?êù?
ºë2ï?°ÀÚ¯Nô¯?ª.JuӒ3FGL J2225.8-0454@M……rÀHj> N¿À8l'šÿÀ;g%ª´t?ñ2KÇ~¯3@F3´7€@Þl ¾4¿à>µÐ[øy¿æOEz³zk¿å€EØ|Xk¿êia1ëæAGNfsrq?ïŠ7ÂåH?†Xƒ?{®[@Ù2?yYQ3×èÌ?6]´[S?ï2.?ì{5°x?¼Q@=,l?œ[•v)x?£†Ð‹‡?µqlñã?·ÚŠ7ޟ§?íßèpǶ?¢ÜáŸñ6·?¥õö·¶³Å?–z>O&)?¨
Á<Ðç?˜=?
ˤ?è3SB=8?·Ôö9ÁËZ?°Å+'\³±?¢
@Ë0£Õ?ÆÐ/±H?¶æŽýïW#3FGL J2227.8+0040@Pw[À6ãÀFמ_Ñ÷¯À9'|üªàêÀ;"},{‰
?ñ±«®o@6Óü–ê@'?ØÝý?äÒ»Þ+ޚ¿å©`ã<¿â¤ØXŠõV¿ëÎQ":èAGNbll?×'™v¡
t?É[¾
žá?Ñ?Ʋ"« bc?×ÀwXÞ?Ê>®h¸[Ó?Ú6k ×?ÇÏÕßó!?Ôª|°È÷?Æ#»4ò?ÑPLä1p?ÁpƆ¿ü?Þ.íã%š?·4q
²?×6ÓBŠ?·ÚœŽ»0Ó?Ņû «º?¨ë)Ÿöö'?ÔÆA(õ)?¸ºRØ¥^?Ö­Ü0Qv?½ޒ=û?ԋ⦹¿?ºóFْØ3FGL J2229.0+6114@Z© b
·@¡àE$¢À6,6*^x[À:tĪ¿[Ë@ž<ÓG:@'3DÐêi@&k×j¿Ø¼˜!I{Ê¿âêÚ»:¿åIÀÐó¬¿ì²Mx6{PSRPSR?*Ç3Ä:?+§õ³K¥)?ïá»ù~À?sïZuM–Ó?m?ÐÖ$ûÒ?sv§B"fº?"0ö¥¼J?;~ÂàÂg?íÏZXú*?±¤*ºaz?±~±ø[Í?±£€‰c"?Š:MM·ó
?†Ÿtpvu?ìEÌW?¤
ÞG‡?·Î‡õh&ã?¡ì}æÜ F?$uàÙ«?.èðnðL?ï•p5€vü?Œ$c–Ž×?ŠR¡ÕÙ?‹·¯_£3FGL J2229.7-0833@KíàBËWÀIÛÒÀ+ԚÀ7¤ä+Ž#À;Hª9$
ü?ùÐÁÙ©ª@‹ÆùÏq@©x3îD¿ä'ë‹îz
¿çggWÒú¹¿é7dQ캿íàP8bÙ$AGNFSRQ?ï´¥×t‡?ƒï¢KŠ´?|I²Ý?ƒváU5á?cÝ	%¾†?cxØ(º{%?ï½">Ёô?~î!3@?PߘD;m£?Wû¤·
õ*?}6ú†°*a?{'d¡h¶?îE×ä?œoBIU"?£ö°šúØ?•¥M&îÍð?"©ûïq(?[¯ƒ¡'?ïtý—óÚ?•JÛ¥,?Y˜²;qw?c¥H˟$?ˆL÷[¬?"®-Mpè¾3FGL J2230.5-7817@st­••ÀB8H˒:À9Eg™TÀ;¤`·Ð¼À«]¥wžG@ؗýZ¬@P_"äN¿ç óäq¿å`Hü.u¿ãL
2ïý¿ë[×ãðï†AGNbcu?ïð·óõ?`О²Ny?<¹üK풅?=øÓÁ­€?Wa™Úf}?^Î弫‰W?ïºK—…î?"D­À)€?G¿€yèêv?PAëO/Ž?ÿj$ÿì?"ãQ>ǵ?îâ|jÅÛ?ØLߏî?Ž…á۔Ć?"	Mºð…?"m¹z;ª?ƒM#‹í"ý?ïãVé׌ó?xAò4[ø>ߒ%':Ù?«A5—?l™M©ðL?x.ÆsŸ–3FGL J2230.6-4419@v³¿µÀLƒT_Ó¥.À:P/žS<¾À<V	!ò¿ã™õ&­ƒ@
ŽYõiÏ@"NàbÖº¿äÌRخǿèq‡DÓ¿Û9'Åö"¿í›oËÑ
…AGNfsrq?ïÆõÛï?züï‰
ð?UéðÎ*?XÌÍ0":?w:ÊA?xI~µ–ùÀ?»7êØ?‹©—±ÕB?`"9"¹?g0Â}hÓ?‡ñBð`Ê?ˆBE×^®?íx)&ú&?œu_ŽÊPÃ?¡zý=_r?lzËæG?§px"Ž"?"f0"á?ïGîp?ì~ "?TáEàÎÎ$?ZugLgY?1¤%Ì?ƒf3†3FGL J2232.5+1143@SZÀ5¯åÀCJ—à[õÊÀ7X‹÷§qÀ;#¾Šêª-?ü«zŒãþ˜@"HM÷"±@·'TU흿ãv-¨Ò*¿ç·@+T¿é¥*LbaÓ¿è‹隸ÓAGNFSRQ?ïÞF	ç›?hÂfê¸?dÐ1^ÏÊ?eÈÃO·ê?YӋ'¶–?Tò܍tВ?ïÁ2k0¡å?}¼ƒ'4!ó?JE»kºW?U×ê Ί?|#A°A—?{w."jT?îm¾›.Éj?šG螲ö?—Çm§¦Dé? .?o?š€¾ò€Ù?'ê;ÕìMõ?ïꟄFl‰?rc`‹?A€7+܁?+R¤óŽÜ?dÎo·Ú¤?r?qdÑî¾3FGL J2232.9-2021@Bºø_øŽÀLÙÌÿøsDÀ:A±Y©¿'À;ϳt62ÂÀG-BÖ¿@×3#žì@¥ùÿŠå!?Ç%£ø%M¿èFz™Šf\¿Ò_½m'Üj¿å+ñSAGNbcu?ïìÄDtÆÛ?f&~­Áž?&)q؟TÍ?,D+
ð»?aÙ$m¯/s?eãæCÐå?ïÆŇ3¨S?9Œ'œµ??Hâ)Óþ­?P°ódÿö'?y  ñV¯?€]l6¢?dŠ°?¯È-´Ön?‰ÊiÓ.?wC
­†_ñ? ¤óÔëÓ`?Š™o>?ï¡å›?œNX'Jzš?YÕKNô?vŒ çP^?œRþغ	ù?œI¦A—ä3FGL J2233.5-1235@I&û?¦ÞüÀKR·?œÎÀ:N(´T0À;µŠª¡¿ü@Hð^Í@z}[‹a@û!_Ìr¿æk½à˜(¿à>Ó	Y)¿âR~WsÚB¿ãº#r AGNbcu?ïØMŸ?vÍû»ý΁?;‡(ÿÉù??2tñW-?r>ƒØwp?vW\Iù?ïÍu2îM?xëÿ/Ž#¦?F%UÖ	?P¶Õè֛?vsaæ"?væ;¥åçß?î4ÝsàÌp?•êAÖMàÃ?"‰¬ì$?ƒ"Wåï41?£*ýÂã?$Û\)?ï–gë‡?yÒæ–ôÁ?÷Ÿ±li}?q³z	?ŠJA%Œò?aú0ÊNT3FGL J2234.1-2655@9N¡¿ØȄÀMÂ'?ßéàÀ:êÛ«ŒáÀ;é"C÷¦•¿¸cðHà–@,¶Á™®@ÿ²}@¿è ‰	Ôj%¿à'<\kš¿äžª|.¾s¿×À<­Ò®AGNbcu?ïöƾ…½?N~©OA ^?:Ñ3Ñd/¢?:¦,'ٝ¾?G|lYuÅ?G~xøˉg?ïÆõuðؽ?}µáZ ˜É?I['ÿ®ª?RwÖÒàé?yYÑW3«¥?{lÙ$ø'?ï'Hb«¿‡?…žÙ­ÞŸK?ƒ—£§±®?tž«-é6—?'K!Ö¯Q?~÷&%ã3?þ¯1L?"r""ß½?=ÿÊ.Òû¼?D_LŠÛç?Žk½x?",¶jpÎÒ3FGL J2234.8+0945@S "AÀD8G@0q¸À9"h¸P>À;ž
§ù®­?ú$ÉñP9Ô@ü¼(º´F?û¶\/Ö²T¿¿aÊ®Q¿Øý˜MY¿ç]RÑÅ@¿íò'³e6PSRPSR?›z4PÝ(·?"£íÓßû?î.zß¼"?­ïXþT=?ž¶‹"+Dö?£Òâ²Ð¿?ϐC€‡Ú?Å(™š´¶‹?Ü¿î牻?Ë" N#ª?ÓxeoX2Y?Ä3xmPÔ±?¯Pþ£?›Ül$=èv?ë¦d?!?©4×zfq?¸2ÅS_ª?¡£C]ÇCý?ж¶Öà?°œ°Á˜?ãh>kãs?µ™ðKYjØ?Â?˜âÅ/û?¯~Á'«m/3FGL J2235.3-4835@u‡É¥ÒÀL1@ìFÀ9?ÿxÃÑÀ;Ï3ÿáÍ?å©1°¸UX@·VƒÁ@æÄÀ8ê­¿áø4Tª°¿æp)Ý'¿ç­;)¡¹ú¿ïÿ§U¢|uAGNfsrq?ïõÙ½ÁgÀ?k½TÁTš?*Ìr‹¢KQ?+|öCÊI'?Pòö+¼5Ç?ko¬{â¹?ïh"ÄHÝ?›TÔ©[Ø	?{êž'"?(8 t'?˜/²ãO?Ÿ?–0ƙÛ¯?ﮡüÎp?ˆy»®Ú.ù?YëCByÍ?}ŸÝ
À?6Äôý?}–*!³]?í¤ï"oz?§Q
áNm¡?"ÒÒ0b7Ž?'ƒÇÀ—?«G°×<#?¤À¤Š½3FGL J2235.6-2319@@.Vßà¥ÈÀM"
Ÿ–2ÝÀ9¥aÈqô9À;ÒaCöÈ?êô³JF†@ÐÎäÿô@‰¯ÀL‹Ê¿æÁd»ã½Ì¿ìm<<'x|¿ã@`óaK¿ï¯òuÝ
AGNbcu?ïö `?S_üÀ}…?1Ô
ٜ!?@;Zƒt½?L•Ÿú)—?NÏñ¿Y?ï(7ü¹¥?™]L–re¤?tB› !?z‡h©:?•èy?'2?•(Ñ}–´
?î{`I¶…?">¨µ±Šˆ?–› öõ›
?‰J‹ºtœx?™øÕås""?ŒŒ$	6€L?퐥²q[¾?§Ò(º½m?Œ¬³½Ë?c?‡#vŽHw?¯Êwéwt??¥ê¤"SØ3FGL J2236.0-3629@	tŸå
5ÀMöWŸúëÀ9lÙÑ.[À;Âßp=½?ܸA_r@á!c|ý@›ú¿Ï8b¿Û™`GØ«¿äø—'=J}¿ãêĊð¿¿ã4dœÈßAGNbll?ïõÍÂFÛ?WüµR }ê?œÍþ7±?Ûwmi~?Rš®'˜h"?WA´âç?ï»W3wý?þ¥˜ø?P˜~ÞEôè?T$¯{ëÒª?~.FŒoõ«?}Œ2=ƒ)?ïE–²¾S?ˆY.Aê¦?ƒ¡°Ùšp?t¡¢vÌÚÜ?•æt½%èb?ƒØúÐÞî†?îþìÇ?•ÑÐEE?Y÷¼­Qöõ?YòÁ-)Ne?žž&£qÿV?•cߥV,3FGL J2236.0-1706@EÌ)ÿ­Ê©ÀLšŒ 4RîÀ:N×úþ8€À;ÓÂ¥+ž¿ôsÎq»@@å""@
3 "ÉK¿á™»&ÿj¦¿ÕTR|¿äÖǪ¿à"²k;|AGNfsrq?ïð²k´Ô?Ux[ÀJé®?=NR%8ÈV?9,¡B|:?WH2ŸH#Æ?S+ý¢GH?ïÏÁ2Ëe×?x'ÜÙ~34?DŽ"m.?N3i…^èà?u'÷šˆ?v"!´YH"?îµ_9H?Œyßfvv?Ž¹GMf?åÿýÞĽ?™÷uWV¶?"Ïàyf?ï¦p¡'÷?|¥#}r#æ?ºzþ\0Û?&¿`L·@º?†$†!ž‰«?|w,bè˜z3FGL J2236.2-5049@uNß°Õ ÀK"î²ÑÀ:,M…>À;ã"q;¬~?֊Ø*ùÓÁ@
'ÇÍ3¤ó@ÚP (êZ¿áéÒ­˜¾¿æÜì/œ-{¿ëïée¿ïÿÝbh¢MAGNbcu?ï€\¦WO?'m"cZ©?`ÉÌÅä#?d&	î
›?‹¶cx8²ò?²ÞEa?ç׊ª#‰?ÂØâçYL?¾UϺ"ù?¹Òiºü26?Áœ*mâ'`?¶™¸èú?ì)¹ÅHvÝ?¡Œ†Ó?©>øôçñI?'"i24²?²µ[HPw?šÑ#	x^(?ã€ê^¤c?¸ºò ·?Ê´¨øÑ©?¶ºøÛÒo*?ÇJë]³Åp?±4µ>…²3FGL J2236.3+2829@V†à€øÀ9¢¬_nû`À7ÛAõmÕÆÀ;.ì³òá4?ø¤Z­ Œ¨@Çj²ÑN@5¸ÜU
¿à-Îy—'ü¿ãbºFÊ¿æ·£®à¿èæÜ­ë`6AGNbll?ï¯WÅ×Ù½?|9@"-ˆ?sáÿy=…?ttð­"eW?tršÕ°?råã^hœ;?ïƒ˅°?}BeäÉ$è?S}+ƒkø˜?Z^ ¹›?yß%¹b)¶?y‰dŠüó?ín£hô†$?£zª]¯	f?¤®Í(3(@?š)'RO¢ƒ?¤füH"us?–7Ý®â|Û?ïÚÂ~_Ÿ?zc³`Š—b?%e5&VÊ«?9L??qó—My?zxr9b3FGL J2236.5-1432@Gñû`^©ÀLßùÐ;À7y#zX‹²À:ÓÔÄ(?ø9ÕÙ滶@ VĹÜZ@#Ì:«¢†¿Û3T
ÑØX¿âQâǓ†¿äZÀþd,¿äØq*\yAGNBLL?ï΅œãÆ6?u"*f¤pu?B°³s,L¹?H9äð5.ò?vg·[?t‹`ZÛ¿t?ïӝBx׺?v²&Î
ý?C™ã¸Ú?PAÿ½Š*3?s¾:ç _?tb\ù:xê?íŠúÆI‰"?¡tr…p³'?˜ÓDǒm?XˆïS²Î?ªæÉùœ?›·ùÛ91?ïü
È ?Pf¾ïö>¡ŸÅK[=n>À²½Ésâ??ÜS#?PcíjÖ+À3FGL J2237.1-3921?âôÕ@"ÀMÌÿ ^¯¹À9§×ÂÊŒÀ;Íiϧr ¿ÙêÍ×lk—@APt6³›@ßß»<¿âCq"öO[¿äF†TËè¿ãèN.Ð稿á@ëæÿ(AGNfsrq?ï÷W'£®?S}Ï&+¥ý?¸ä—?½¢¢gÒ?OïºÈ¥¿=?R¼-×àãá?ïÝÅùðá?ròVÛ]üª?9v+>6?C]8#'ª?o÷J‡V9?q©
ÌÞ"=?ï4ÂEfqÞ?†)QsÛG­?|AøµÇ?mT•…ôï?'f§
ó–ç?ˆÙĉ
m?ïô:ŽO²?X@i'—¼b>ӊ'úç©ö>àÁ¥rj'?WwXÝ ø?X9NAåa¶3FGL J2238.4+5903@Z£h@[9â?ޝ¢ŸŸ›À7±E‡ÉÀ:²›ÉÂ@3¢x:yN@Wúÿ'?þsÆV;¿Ñ–·÷þ~Ì¿ãÈ´˜p¿çìÝÖVÛ¦¿ì›R[ÂsƒPSRPSR?L'yóE?GP*¬$¶,?뮘øy
A?Á­¿¦üR?Á)¡ã¹?Á¤ìid·Ö?Y§±@7ÈA?n=vz¯F%?æ=@¼Ò½?ÈZobAґ?Ól%ÍF"½?ÈRa͕È?|[ïmN?xˆ	B#¼Ó?épd™Ô«?³R²/K"y?É[Ž#-Bæ?²õ¶åš«?ƒw¼v[£'?}‹ƒ/øFL?æòˆ™‡?»J6Äã×á?Ñ(;ïÕ?º¯P©(m3FGL J2240.9+5831@Z¥ƒÑF¿Â8ßowîÀ9•ÝŒ7±GÀ9›V	÷Ї?ú±¯ÀL‹Ê@¼%†¢F?ìêŒèé}¿Ïà'·)ø?»Za»¿ç	'6½›¿ïÿö¯Á›ŽPSRPSR?WæŒÉ÷5‹?iäx8Ù'?«U¼&†JÎ?¼T½P°
é?î>°÷2Ÿ¹?¼}ä@¸?ÃߞŽ ¥$?ЮO7ÙK?ÀGõh»!·?Åo1¸ƒ?æö)I?Ó'$`þŸl?¬³Lñ#S?œy/Žõ&¶?àwÆÐÞ÷¤?²›*rõWÖ?ې;ô£ìL?³'2™ ?¾§½¾Ç|Î?Æ,2?‰Ïì?Â܏VÍíf?ÆmQ93ôÁ?çsärs•?Ð->ûabÚ3FGL J2240.9+4121@X‰}ßÿ¯xÀ.Oç_JHÀ:¿k»9ýÀ;|Î>½¿»x'b@敠¼@ž2 f<u¿ã\ûn¿ëT™¡ô~d¿Ôû¤åìÈ/¿á.»c\µ|AGNbll?ïo*P"­?"Շݗlé?3êT]vX?8«ã`˜?'Ë±ôt?"£«G
9­?ï{2Œêµ?"2²T׫?h܏Dn
W?pƒ1ž&?Šü8ô^?™Bò@Ëè?îv©,(0?•¹ÙKi¾??‹Zt¤Ï¦?w
0ÈÑÁ?§±øD	"s?'´ÄžóîO?íšFšzý?¯ï+_hÖ?Kƒnœ]™?RäÇ ??²öÄNï]{?®ö÷§8—3FGL J2241.6-5237@u®6	ÀKuJÞ™À82ª§ÞÖ»À;ný`O@N\Õn@jt#"X?ü‰ïµ…'¿Ð©RÝ{#j¿Ö¦˜"Š'"¿âÚ°E‹-#¿î¸R‰åœ|PSRPSR?"Ø À78?']ªÞðoá?ïiÆO$Š"? ÈÓIԞ8?€µÌ$#|?"ö§²#5?‡;{E®R?"®…ã?ìqՀã²?ºc=Q¨æ?¹‰ói~ì?¸'ÞÊ	ÔÏ?©÷0ô3í?Ÿö¾ã‡»?ë³gÌÞ÷"?ª{¨îV?µ¤ÆŽ)q?£‡Jéä¤@?'Eî»äÄN?‰>ÑIrq?íæ¯A¹"?¢ÂqFFy¨?¨ò'BŸ?Ÿ9û.ªo3FGL J2243.2-3933@vyÏÏÃøÀNW³ S\žÀ:eÄ¿¸TÀ;ð^VÀë~ù°/³@/B%¿W@ò«]ä¿ç—™‡jÿ¿ÝÆLM" ¿è¨šSd¿çj3;°tAGNbcu?ïÒµ'¬zX?u!ӅÂÿ?bÏa2½?j£æ/ñ҅?j{vòS‹ß?i±mƒÜè@?ï«%éã#¹?œ‰ÌÃæ@t?Uêû
I à?t,ù ê±?'y&%íí?—þ_
Â'ˆ?î^1Íh?"¦ŸÃÁÆ?—Í|ê?‡?†õÂĵ?¢Z7®Ö4h?˜âUœ?ï|ô_G"?"NÉ·æ?%my›õêl?@<eD*¹þ?6™Ÿ!}?"8JËß3FGL J2243.4-2541@<t/ ~û‰ÀN±W€•ÓÀ8¨Xçø¢>À;'Ì؋Fð?æƞ‰\Ny@ö˜Ô!Õ¾@2¹@(<¿á²Í¯m7Þ¿ãV'^o¿ä~v"T#¿ê‰2°Î¶ÔAGNbll?îŠNAèW?©–ëTÐd?Ÿ_¢é"?§0¯ÊdcI?dnV@Ñ?'¶`»-u?éÝ DÁ¬?Çä-»\?³¯("?º±ÊB*µ?¾N±s¯?¾aŠtq
?ëHºL"Ñî?«/¬Ù®w?µ÷>nlè?¤Ã£tý@p?¯†<ºÖK?˜ƒóß9~?æ'(üùr?» |ÒCÃ?³
Ê"?¨ø¨ï†?Ìn†µ&­?¹pý1®û3FGL J2243.6-1230@JRe?õ¹UÀL]â?û˜'À:%©|e¬,À;ÁÔ2Ûÿ?Ö®ãû	£@p-è±@ÀÊ+¿äG.B¼Ö¿ì¤"{ó¿¸Pí ‡èu¿ÖãlØ׃AGNbll?ïãÌj°R?µgþôãš?4ùi1¹Ù?hIM®»@?ŽßDâ
]ä?´ÑWÉOÜ?ïµEòù'?'IX[[cC?Q"ô¢cÆ?Y(PD7Ò?€}äùMiu?€~ü5^áÐ?Րª}?Ë"¢V+Ü?'ò£Ñm?qþ]v©%½?Ÿ2Ã|ùà?Œ'_Þ[ÄM?î–âãö(æ?›a¹×è0›?B§VB(?T­%B¡e0?¦IÅn?›[<d´13FGL J2243.9+2021@U¥Â # –À@®(€QÉ÷À7³ŠÁéÀ:žoStò?òý>áß.@QŠDg
*?ü¢Ù;(ö¿Ö"÷ïÃÐW¿Ö'ÇɾᎿÙüÚkÆ̈́¿Õ¢/ÁIòùAGNbll?ëJ"¥""?½·‹C©la?ˆIFô÷k?‰Z¾ÒHäs?ÁQúq R?½DU@Ó²?íúŠçs:?²²Ñü;§?‹è¯M›­A?•qX:P?©]%µha"?­6]å?áÆ2	?º'u rE?´m×ÿG­m?Ÿýà¬)þ?×X%î-s?¹ØEµ<?Û¬©×\y¶?ºkfhšÝð?¢'VFHÅ?£°ÖéëÞ?áþí^˜?º>hÉë3FGL J2244.1+4057@XŸ£ÌhúÀ/"yÞé/À8¤zôŒÀ;?ÜìՁ?êÛBG'þ´@ë¸x¬äû@POŸ¥wH¿Ö¹k:p¿åT|/6µ…¿ã¶C¦üaC¿å'|/Œ›ÀAGNbll?ïð©1w¡ù?S~Øü[ ?B¶R[Fy?;hW½û?URsãµ?P¦‡´©Ú?ï¼Êã²'?'C°ïì?T6~È´"?Y²½ÊÆU'?|Œîtљý?€¾Å{Á­"?îoc8Ì?'üQy_:?"{0¤»?"áž6Pò'?ž˜hXk?Š,"¥ºˆ?ï¹JT%B‰?€ a}rØ?&¿ª*§á?0.½)³Óp?Rlð³+?ï,xâE{3FGL J2246.2+1547@Túâ€'،ÀBµâ (zÀ9•9"†À;<L$ˑ?çgØx@rP@Ùå_jÉ¢@v9à¡jô¿çy¯nm¿èû#½/²¿Ü'øª˜'Ô¿Í&hä3àqAGNbcu?ïçX³ä§?n=]"B¯?*_ré?7-ó©Lð`?fþV+ª+?m.Ì×0`?﮾A8·?€Q Žu4ƒ?QŸDçg?W¨›Ä{›ñ?'Ž)[U€?}›zeÖÝ ?ïÖu `?‹'éUò‡Œ?~©o
±X®?s4Љ?–z՛Ë?‡N~g$!N?íð]Yޘc?¡K™¯IÈ`?H˜æâÌ?UaŠvn¯v?°KãcE¤²?¡.ð¦bº3FGL J2246.7-5205@uFŸŒ!âÀKí: þ¡À:-¼ÎRÀ;ƒìŒ…´à¿Üœ²
™@
½Úg•œ?÷!ÀD(N?ïñA2œ¬Á¿Ý+$Ÿ$P ¿Õ~uh"EA¿³ÔꎺԎAGNbcu?ï¡t˜ª<?šu-¡ïJ?$ëŸËò?+m¬ç»W3?‡i'-nñÊ?šo|fƒdú?ïÐÁ<ík?w‡ôNäƒ?F7$,ÀÉ?Pm\M.¼?tØ}Ú°R?u;y(oæ­?îoԆܤ^?•MÊõ³i?"¢<á"c?Œ6Õ
jóN?c2B×Ì?Böóâ6?î¯à`¯w¤?˜šrétÿ?Í4r
J?.Ã/[aN?¤ó"nîL¯?˜–Fým}Æ3FGL J2247.8+4413@Y-÷ µíÀ*€Ô`?ùÀ9¾P"–JZÀ;}ð·Ž?Ö$8'¨T@ "=¼Îþ?üºÊÿm3	¿ä‰?ðcˆ¿ÕŒ¤‰óÅp¿çxíztîÈ?ËÔÁÔiyAGNbll?ï˜Nk¤á~?†uK>6ÿ¹?sB³²ý…?u¹j'¨Õ?€K=Á!|?€«ô4q"?ï ½ªbG¹?‹cCGê?]ß×ÌgÚ?f%ï€]Ò?"šmáÈ?ˆLDù~p`?îWÔèì‹?"#7~Ì	L?–™yϹÙõ?‡¯TP;†Ë?žkí»(" ?‡PÌÇ»¯?ïU}7Œ<_?'le~η?LG쨄/?]ªºK{ü÷?"n ¯/õ?'.~ñ`Q»3FGL J2248.6-3235@+}ÿ	_ûÀOué_ªŠƒÀ:ðôÊAØÀ;ñ9F¹?Μhv66@+渱7@"à{*n¿å´ŸzÀKÆ¿êD¼…Vìv¿ënL´cŸb¿ïýðõºÆAGNfsrq?ïäÙ°d?}$2Wbf?HòŒpG"µ?WÅ&Ž¶[ï?e§ƒ3Še?wÎØM5jk?îpElÆm±?¥LJ*PÌ?†íôï/‰?‰ðÔdö?£@+÷ÍB­?¡ù´"|¤?î^³t¤?'ïØHA?˜ÍÀóma?…~õÕÆ?›[Û¾uþ?†k&ôõŽò?노ÛgR?°Í]DH·°?§«<ˆï?ž´)䪯?·ü›¶§Š?«‡õ~àðV3FGL J2250.1+3825@X²à'¤À2']ŒúÀ9(&¶ÂÀ;WD²·wÑ?Á½À´æ|@¬ƒd?þ˜¶?l§s¿å°6E®­I¿ßÁpïg'¿ÞóSãñ›¿Ö2t}xAGNbll?ï^*iuÙ?•ÏµÚÆß?b+¨ý2É?`σ|á~?'ú
\<^Y?"ñ€_ï?ï`ïŒ÷+n?˜nV@¯J?o>Âaç6É?t;'XËÖ?ôl)»VË?•@,M?ÈI?íÛwKÇ4U?œ\ÅÜܕÍ?—8oØ
ò?‡–#c'«?¦¬SWˆ³Æ?•µLIF_?íg^ÖðÂÄ?ž1…è÷›C?d0Ñ¥Ÿù?eBLŠ@?´$ÇÁì¼ç?ž å5°3FGL J2250.3-4206@v"Ÿ×¡<ÀN"¢¿³ÖÀ9½Ì'ãtÀ;À4"\B÷?éž©4'‹@³-QFï~@D– "Hr?î?Þù[\¿à5û×ý,'¿âžì>Ø¿èj'–qñàAGNbcu?ï¦JX$$?£Ó\ãâÁ?ƒ°1‡|{j?…ƒ(óÅ­å?•óñ==Ã? èÄì;?퍏ÄûÁ?°¬Ó8¾š?—T[tn?˜W°´Êù?«¥Y'‰·ó?©¡ÍK(rŒ?í¦é#¹š?Ÿß•¤uÞT?¡Ž÷1ýR?"¯Tþààä?¤Šà'i?'ŒÈÍdÃÚ?牂#6"?¼gÈÉÓå??´Ð,{?¦ßâ4ñ"¨?ÇΏÙgè4?¸Ïé˜PB3FGL J2250.7-2806@7½f@¦¹=ÀO§¶€Z-sÀ7ÇtZÏYÀ;[^Ëgr?ï½icà"î@
Ő¡@k(_ššK¿àT¢pN¿¿âûØZœë¿ã õyÐa¾¿å¤ÓFíÿAGNbcu?ïò9œM"/?YuÞ?-®E?*~Ø:Hñ?%°Wcwú?X<ì]4?XÁ«Ò?ïÎlWðh&?zc²pÕ*?F¶éL˜¶?QgJ#O:?uòöÔ"Z?w…$Dþ·?î~ÅÚ¯º°?";ï¨@°?‹ôgé
Âÿ?iÅ֑… ?¡ˆZÁ¤K?üÝh	]ô?ïÃÆTVõ?|ÙÖ!'µÙ?þåàL	?½¬3ˆÀ?}Üÿ
í–?|ÈÝü2qL3FGL J2251.5-4928@uJ^`=WyÀLú`à¨.À9³C½Äò
À;¶V¼¥7]?îyù$]q9@©;"@?ÿx®àR»¿âzï(‹¿ÜSLÙ!š¿Ô§RR:èè¿ä%ržê!®AGNbcu?ïAqµÕ86?˜*ÛV†"?n[öŸRß?m¶ÒUâ«?"J"EÐ?–íÛzaÆ?î¿ûäNcz?¡Š9±y?€î=oâ:¼?'â*³˜9?Ÿ‰d¾Bsf?ÁU©<_;?ís£µ"Ë´?¢ˆ… «?ÇwY4?å×¢!'×?©â	º#?šƒa_b)?ì	Èõef?¦>óŠÇª›?"ÑÏçUB?"«,E'U?ºòDZÿ~?¤Sy±Ò…3FGL J2251.9+4031@Xè#¿ø¨ôÀ0àé_ªŠƒÀ9:$)ªô5À;‡Æßî¿ÓH:õR¸@Iá">éu@þh`f¿äÊD;œ<¿äW§¢¬ùÚ¿ÙéO¹?–¿éí'u¡ÓáAGNbll?îÿÊüì'?Ÿ«gȹX?~¥
ñ)"?~!ƒ{U?˜]]üæ%o?›ìÎ3š £?ï)ìdÙX?žê;CàÃ
?x»ªÃÙÌ«?y§ÿC`Ô?""ˆ³Þ‰Ó?›oU ü—Ó?í«'ßÓ?¥PC"¥¨8?¦mEè\L$?š¬]94b?©(ö¶Á?–-êÕÔWS?íüì?gRL?šØ¬á£›ò?i	zZ£­Ã?g>-"2÷?® ¤cà I?š2j‡ÃŠÆ3FGL J2254.0+1608@U‡Å_ñ_ÀC_ÏspÀ4ƒJïèZÈÀ9ñ´Ï€t@7PÜfs@&LÉn¯?ÿ¢F…‰A¿áÀìªkV™¿ædˆ­ZŽ
¿æ˽ eí¿ë§òX*A%AGNFSRQ?æ¢nTӄ¸?Ìùȃ¥˜,?¶@ÿЁ<J?Ž"ÝãC?ÊUÆÄqNü?Ê<3àc	Ö?ï¸è"ÕNÞ?–B™Ø´·¦?_93Ö<?‡ÀeDÃW?{Æ'UK›™?¼®R8
?ÖBd£ˁ?µTLI°?Ñû"ÂMª¿?¸Å;Ãr´?ךŸ‰¿?½¹ã\?ïþÏKëB?JFfŽn>Õ]—\¤!?ND³É»?/H"Ðú"?J'õIõó	3FGL J2254.0+1403@U'‹ŸÛÒúÀCõrØœÀ:0<îÀ;aC§õ|ï¿àõÖã?ïž@Uö÷Îÿ@ì‹àžeÜ¿æ4»ÚåÄ¿èÖN+î+¨¿áô%öø¬¿É#ò)ŽÖAGNbll?ïïÙ̊þ¯?dB@Ǝj?'TÞ¶Ò°¸?0ʶ.È0?]aË(Kµ?c§½×@Ó?ï¾ÕޖU¹?{#ì/³×p?H»ð‡=ßå?Põ´¬ñd?}}'£ígô?y=Ë®`•?îúëþèî?‹óIkY?€ D8™«Y?skYß{Öª?˜R^°Ì¥?†ozTՁÓ?ïOU҉C?‰ ¤m¿°?	°D§¶^?qá`4Ì_?–‡[ŒƒÕ?‰8«dû3FGL J2255.1+2411@Væ æÀ?ƒ:€.Ž‰À9_h-æÃÀ;€·Á¢Í¿Ób:h—Õ0@Œ—[Pޕ@'ž‡t©¿Þ€ÔñßUæ¿ÏÁô—1›¿æ:'Dˆ¿Ú™ó¿ˆt6AGNbll?ïì'ä ˆ÷?hÙ¶ëßn|?:÷*%üøV?>!¥¨âÝ]?`6·k,?g]¬¯?ïÁÄc2æÁ?{©¥Î®ò?N~»	©%?R
,a}Š?{M÷W{A?y(VwÏ÷?îŸÔ'æ[?'Cۄ_á"?"©‰u¾%{?‰€(*Íì?—[äJ%(?†~
Öݘ?ï¦ÌÆä)g?
&4«©}?,|K…Uím?3èV9»?…ÚÝàN·?~íNKð
Ê3FGL J2256.7-1022@M›Ö_ó…žÀMCÀI0ËÀ9˜OYÚféÀ;à,/2ór?ü
߬ùH@¸åå!­?ùrLK:\?íN'˜Œ¿×lôS¾1î¿æ&äv?U¿íšpÙÃPSRPSR?x4M*¢Iu?"|óã'O)?î"_ÿù?´.xùBÓ ?¤³"šK·'?²úÎ=³<w?''"#ŋ?£^
¼æ×ö?ëëÑC)"m?À`=‡€S?¼…Aíû0?¾;î	ò=ž?´Q•Ìe? ß"ÖÁr£?é²ù•9‰?°¨Z€åe?ÁЪQà3¬?­IÌb"'¶?—µC½àÿË?•sûSª©?í£W(_†?ª¦'îàŸ?©ëˆ®‰‡Ø?¥-M84t¡3FGL J2256.7-2011@DÈL€SÀOt?Àà0À9HÄIpŒZÀ;—¢çöô¿¿âíÐ.q~@
/óf¿|­@½}ÿµ,r¿Ý}Ì¢8,J¿ã[úk…¿ßp÷TñÛ
¿ä¹±~AGNbll?éÊÔ¡#V¬?Ä3ºÈÈä?ƒÆÙ¸K?–Ö­i?ǘ?ßíôÝ?ù7ûuÕ°?îW¾Q€|?º€Üæ²í?…}î	?™¡M:­µ?¥MÓ|Â?¶,
xæD?ìx™ÈÜT?¢¹Úv˜«´?¡)^0'à?ý̾\!?³un'¡	i?Yók¸s?ëEWf€j?±EĬÅ?r«›<š?q%Èc¯z»?ÂZ#	$s?±ǕX¾3FGL J2258.0-2759@8ZÝßCÇÖÀP:B×P´À7¾Éãä@‡À;=ĵ§Z@'ûE[(ñ@Þ%™Â‰R@øӞM2Ž¿à¾o'Þ9\¿æ—ò_®fZ¿ç:c‡Jë¿íD¿ÇžPAGNfsrq?ï–~:±ê?‰€dy}?…HNw¨g?ˆ˜Z¢¹ÿ?d`‹q«Dõ?`6-V)?ï½Î©†?ˆPøýÁä?T¦3ú8?tqNZáÞÉ?{ïj,Ôo#?Q¢YxÔh?ìil°%ã?©ÜÙÃ{d?·i*²?¥ì/Dla? R–ß™"±?•úÜ÷"?ï¯~"F?ŠZðy¬åˆ?Gõÿ_ÅyŒ?`¬0 Dsr?'¡äþÙ?‰¿Þl'
3FGL J2258.1-8248@s04ÿ†]}À@³€ KÏâÀ9‹pd*À;vx†?Ò±ó¸Ê@ÏZs@ŒóŸŸm¿£q³üª¿áÙþú±7¿à&Ì¢Qñ\¿èUj3`»¾AGNbcu?ï1˜ì™?Ð?•Iñ =?x™…^ji?w˜yüõÒ?"¦Pëx?'ª@QA™?ï2Wï›[Å?"#	q!°?q{Ž	à‰á?qƒ#¡·"j?•VŠe?'¦",Ï(?íÈZéüFÓ?›¬ÕJjÌÐ?•ÉÄX{e?u›÷öœ?¤¯l~U?'
€›.±Š?ëȨॉÎ?¡rË´0{?‡jEfx?xÍ,þøæ?¾ÍuR&á[?¡"ФAV3FGL J2258.3-5526@t®÷_²íþÀK'¡ ÏÀ:zi
à"SÀ<ë7@?ÑòG" S@Ò3>íÂ@|®¸'¿æŒà/¿ç[î¤ý"°¿éÝ=K˜?»°fQvHAGNbll?ø¦*?'tÖþ²NG?<Ê<t\Q?Õ}‡P8?|7äÇ8ŽÍ?~Eín?ï¦ñäkk'?'-yt¬¶?WÑ,Og?rx%ìN´Ž?ƒIfÄÿ•¡?ÀÇȏ?îeeýþà{?"‰h3~åœ?'°ê1C/??…"ʹ'õc? Q+p`›?ŠÈ£¤"?ïƒwCXš?Ž	€Lˆ?Hžth[]±?Yx‹Àð#>?®ºè¤#T?Ï²F?¦3FGL J2300.3+3136@X5 "ÚÀ9
¿v¢õÀ9Eˍ1¬JÀ;df\Ukl?òˆ–i¹W$@¯¼EÀÿ?ý™ž>ÄáÇ¿ãŸM›lC¿Ì-H"÷Ò¿Õ-	²u!"¿ã~bª€WåAGNbll?ïi_ Þñ ?'Ñ!J®ãÊ?mD–wa–?p}IQÓ΃?ŽVòC忉?/aï»í?îÊ«i¹´?¡Dþ°–‡'?†ò>üÉ?'Ÿið"‡?›1.yË?˜ØúŸ§a?ì¦Å§º;?¦(WC'ë…?©ÉIt­Â•?›ªHDÆZ?«ÊdÀ֙ª?œy£·«²L?ìƒD³oå+?¦¶ßvIc—?"ЈŸË¥?"Y<OÜÀ?¶ñ¸<ŽL?¤±ü¤.B3FGL J2301.2+5853@[Fú>¯h¿ï'DŸÀ9Á¾òïvEÀ;:9%»{l?ò³ç®O‰*@åÆî¼a?ø7¥þ׶á¿Öæê…Dwÿ?ïþzÄÂ<P¿ØŸa´ü¿×Á›@bÇOTHERsnr?æji©éw?Æ&=ÃGÇ?»ù~܄ã¸?¸RQ-Zâ?ÈY™êˆH?Ã"Y0Z‰?Ù@ªœ¹¶Æ?ÕÚ¥~…?Ä‹SEƒ?Æ—à•#®?Ü»¹Å¦z?Ôl— ¤U$?ç31ÓJ)¢?°˜5y›«?À»9uš'?¥¯j±ðq?Âwÿ==;è?¨6œ#ºâ?è7nU ?²?¿ƒÑh–V?Çwµ¬º¤?¾"ðÝU\…?°'ë¤)?¬Þo7à²Y3FGL J2302.7+4443@YÙN wmÀ+ù¿è,À7ý£ª"" À;L(T²ß¼@-ù압@h´Is<?ú'òg»ü¿©ÿP¶.ƒT¿×ÿ'¶•B¿âs~õõ¿ìß²ÔPSRPSR?d:™a	rg?pêˆøA´?ïØT·OôÏ?z{>Ïð?cp¯O¾R?hȊ&¬´G?bv+$¡W?€…¿yèÿt?î«:>C&k?¨ö-V?¤$ùiƒƒÓ?¨S›Çْ?"߆"ƒË?Œ->¥
Ї?ìÈî½öKÎ?¢!Fʳ,?´€Å.¨€'?žg၃tˆ?wœ¥·I\¨?qÞŽK F?îõƆxŽÊ?—§3Ó½8w?›`Ãϑ?•†nzv"3FGL J2304.6+3704@Y^"ñÀ5"ÿÖåUÀ9q¬'$ZÀ;iQÝBeÖ?Ýí¾jŁæ@¤Ô…'ò?ýÀŸ¿äm½å ¥Ÿ¿çÇ"5¿ÌèZ²Ì¿²<´fN"ŒAGNbll?ïñá=ât?sjgûș?9g¡û?x?s-A6L¤?U㛼H"©?Qù
ۖÁ?ﲔO-Ð¥?|Ç㨤';?Y~ úµ¶?]+ð—B6?€+)l€A?y…îÌÈé?ïC俺´v?"ŠI
Nó?wœDÉ0ò¸?r¹ú"."*?'œVÖ]4›?aۑª¯?ï;>¼çÇ9?'Ò9?)oÉ"!6??m‡ÞÄp¬?˜eHÐæ?''ïËô3FGL J2305.3-4219@uîCÀ~à±ÀOÎ*ŸæºµÀ:ßNG‹¯ÌÀ<]û]Ùпê/wAÞzR@
¹µ.Ëo€@b¿g£¿í ›:¥å¥¿ /-¥ l¿åoº 9¿Ú]2p?®AGNbcu?ïÀQ6l`Õ?¨—qt_v?w'Šp?¨^9ææ–?a`Ä}?`Š"D¨ur?ïÈ.=?xÒÃ×Ù­Œ?G˜ï¶Ä?P†"–w÷Ÿ?xõÔê w?w=¬K¦6?î›ôSŸ õ?'ÜM²e$e?'<bÎO¨é?ŠËƒ6G¶R?šE½¼8?…%uÇe?ïÅÌbÏU[?r«61¨Òß?2¶{ðÛð?7;+BÐê1?{îfÙG"Â?r'{ràœE3FGL J2307.4-1208@Mµ?Àà0ÀN±v_Ø­¬À:‡kþUÛÕÀ;Ç%l¡¿Üø'y'Å@q!Ôæ÷›?üXFÀ®±Y?è@wO€¿åFðqdÆ¿èC,f ¬"?áQoß6öAGNbll?ï¤?€ ?'Á…°G<.?HÓ®k¥"?QÍb6ø…?…oõ9F]è?'‹"õba?:ÅÐ^â?'v¨¸­ÒP?L½ï›¥ó?j6m]?~ß4]À?mýdĀ?íÍY×þ
?švÀÊþé$?›†¼èS³?r¾L{_?¥¢õG?'¨<Œ»Î?ï	*ñF¥?Ÿ?ö'ótÇ?4"bÞø¦?Qؘ+j)x?žNfK¯˜?Ÿ3þ¹œ'&3FGL J2307.7+1449@V5X`fÀDŠæü9¢À9ñÝ'ŽÀ;gÝX5K;?Ï$¢v·íB@lÏ$ÀԜ@èj#ç;¿â}ˆŠ¿â˜@URb¿ä¾Æ³>lˆ¿Û³ÝF[rÜAGNbll?î"É81?è?¨ÁìS¨£?{þ½w®#?}~
Y€1?¤3œ…=Ç?¦y"A›A®?ïVUþ†o?•ÌR$T{?h§(dÓ´®?rDÕ!ޖÙ?' [0´»?' v¾ùêÏ?ìОœmì?§ð Ë"
?§žÁ¾zS‡?–z‹{k{?³š+ßfß?ŸÙ‡2ôÀ?ì*A$¬ï?¥Q¢Ñ6 ¥?}"1|êã¹?~6ø‰êEv?¼Öªßê>?¥I…TÂ3FGL J2309.6-3633@Cï@j(hÀP ½_ÜßjÀ9øÀysžÀ;­›÷Aë]¿ñsCÄzï@]¸šºx?ý«¢¥é¿é«FuÔG¿âÚ2ÚKæ¿Éð'ék¿âD.ŒÊ*AGNbcu?ïûä'L?DÐjÑ]¹–?fÓ…E?ɉZý?>n"ó"?Dg÷ÛKŸ(?ïąCÆÆ?ƒ\€È\·?EŠ<åø4:?Q/³§q?{*Á]–¦?'oMÀNù?ïl"]Gé?€½(U=ƒü?sÙ/X™îN?bK3ÕVxh?ŠòQëNì?}ÙµE¼¬9?5U?"=èÛÁo>ö.C-:²?Ш¹«
?ŒðŽ¡Qj?"7>¼hÏ©3FGL J2311.0+3425@YPaAcxÀ8_€™"À7‹áP°À;&ûL<µ?ûz9.Êó@3¼]éÀ#@㶿á™üL[7¿åWʯï¤ò¿åY‡lÀV¿ëÌkŸÐRAGNFSRQ?ï•a6BÄ?·ïuwá?…áð`õ"v?ŒE$n"jÑ?c9g^Ï?b<˞G[?ïÄԄӋ®?|™Ù‰–?S­NÛg?Y3›¨v7'?xªzƒc0?x¡º• M?ìâ¿	f=?¥¦†ò
?°Ô³ŒJ?¡%z›)õ? *îs‡?"UXÒN?ïöWgàŠ?c'+³Ûó>ÿá­ÞxS«?#ñ\—¥'ô?RÑ©‡rÈ?c_'õMˆ¨3FGL J2311.0+0204@SÔúÿåþÍÀJ
@TƒæÀ9ÜàáVǍÀ;Æ)}§ËŒ¿ô
ý\aªÀ@d¿o—ª@+b€R˪¿Àâô:"¾}¿æÕÝCßË$¿æ˜	Œú¿Ï¯7¼AGNbll?ïìýÙ%?cŸ"!<Ä?Bç®Æ?Eµ¡ºp?\÷EÍÝØ??be	åªó?ïÌ],ÖÊh?zÅþ«§"c?Eɖr7?O¤€‹Xáb?w6ÆW¨f?xܘìö4?îÔðé'qâ?ÒyÈÂ]h?ø²6%«ß?…p¾A×Æ?–e‰²¾í¬?…`Wev"ò?ïКã!ª‹?t|zŸ£>ê'\m7ë>úõ
(r™ý?w¥M@ô´?t8ŧÔ÷3FGL J2312.9-6923@s¯£¿ø¨ôÀF®v?ø="À:Ë-œ}ZÀ<	،°?ã›U"Iƒà@
^,±
ÿ?üÝK?nå¿ïÿù?Ð??ïþÔè‹Uo¿°œ§W¿ä8tƒ4¨SAGNbcu?ïⷄÞL?p
wÞP÷w?B"NTìXF?D}»?umÚ?h§gŒxç!?n@Gøk›?íõ§?÷ôð?¯Ï~?'šÕG^è«?šÏl3ӛ?§Ø!\Ñ<µ?§©BºÈ5y?â‰GÊ?'dï.N?Š‰¿l«æ?zh+ .?Œ¾Ï °Ù?Ùš€ù3??hð‡?¢
¾›Š?œ²î¸§8?ðŠ0\?'Yd)mß?"dwØ3FGL J2314.0+1443@V¡ùŸÿhÀD÷"ßÎ1QÀ9Ž—rwì¡À;f"Ú<ø¿ðÃðBÛ@Ýá"êµì?ü \†ã‰¿'îâ:6 '¿Ôa÷8R¤¿ßï§yu¿¥Šòóä$AGNbll?ï°òÐ+ŠÂ?€uûã-½"?T›éfŒÞ?UƒÆA&:?/ê÷ð}å?~ÐsFÐ?ï¨ù°(T?x#Ü>«ò?E¹ÂÿwýE?L‰â~n´?{ôJÇüÖV?v"au
8H?îdJ4‡š"?'"ËôÈS?"‹K`Æ3?ƒ~>W³q?ŸënFz?‰˜Y" F?ïHgz˜p'?Žò§ò7?"©É¯?$Z7?–ä
â	:?ÿ;oÍ<"3FGL J2315.7-5018@tê ßÞøHÀNAY@
6IÀ9»˜"à5À;Êd¨ E?å1®v©S@
ÀXr‡ÜÙ@†@.l?ï+šeÏñ"¿ÞtXÔ¤ÔÙ¿åmÊ"Dñ¿ëÒºŠUAGNbll?Ü\Nt;4–?ǨòËa`?Ùö½à)߀?ÇøÕ*¦L(?ÃYçW5×Ñ?½Ô¦® ?ãU%B¥Ñ?Ìl‰ãgé®?ÌïK–?ÄE$'†%?żÝÕS¹?À\/Ìd~?æ­vØ»?°wmÕ܈?ɬBÊ	Õ?ª3Æò?»îÅ-&}?£JÃz+¯|?Ûþ~K˵ë?ÂýÀâ?ÕÇ?jIØ*?ÂãŽ%Úñ?Ìt""ÔãÕ?»S¿¬§3FGL J2316.8-5209@t¼]ÿÅGÀM«t`$-À:£\ŸTÀ;ޏ±¹K¿è i6ÐK²@jîªB3V?ûÂ@&¿èó(!öñ¿å
m*È"¿Æ<C_½r¿Ö§kŸ‹KAGNbcu?ï÷{lеz?Ubò±ZSh?Ã;x£,K?f×÷4a?Ps'Ïòš?Už€±ß_?ïÄоÝU?äeâpE?H½@‰r®4?QÙ=Üi?zø€F1?€™î8PUz?ï^2õb"?òyWý¼ö?zÄZ^ÂÓ ?eKâób!'?•£#	¢úÜ? d–M²\?ïgí	,èY?‰ö×El99?ÜYzðŽÊ?VAÉ ·†?'÷p­¥|Ñ?‰ôXJ™¶Í3FGL J2317.3-4534@ua›«–òÀOà§`+¹ÂÀ9kÝ3L]§À;²ýî­È¿Ê$Û
ŸÀ@â%¯çä«@}1ÿò¿å"¸#G'Ë¿ä5wãˆÈ]¿×iØM€Þ¯¿åD;8?SAGNbcu?ïØjbs²ú?yÅ
ÍÌ`K?.MRNÑB	?/¢/d@??rØd3¯ù?y6DÑÔ?ïšÖUGq?Lwæó?Y0¼;ƒµœ?dW8ÚËJÉ?†$S&Ê-?ŽÈp¹áZ?ï)µ'V?‰F%ÌÓ¥?zâo¶­ÿ?i~&ÿ°}'?"%mpÍÉ®?†+øúÖd¢?î梹Y?"Øw6*ãÊ?DÃـÇ1+?EµÿEi¿ø?¡BÐdͺ?"¨-_ø§3FGL J2318.6+1912@W£?ãDÞÀC?N™À9ÍS¿šµÀ;´¢Þ¼¹Y?à}Ç2÷v@	(ô@P@íÊà
œK¿èǚ´Tc¿èMÎɍc¿èúœQÀù¿ïþŸûˆwAGNbcu?ï҂Š¾8Ô?s".9¿"Ü?dðC>Vá?dCbWU­?ik"þˆÖš?l‹•ÄK?ìoÑ
tôï?µS¿²C
? ¾?£4Ÿý?¢ÀMÙ{'?´"W¾?°",'?íàÖ‰I<?—@ßVû? ƒKA²Ò+?Œ½$ÂÏR¹?¡s·U¸š?jr1?é2_)ÎÐl?°p_…=_?µ>QBx]?¢'|Mª?À—<°#'$?«•
_4 ¯3FGL J2319.2-4207@uÆ# ƒ˜¦ÀP|Ù ,Æ2À:7_èžÀ;âØ+¥ 8¿çG²,s¸@g0¨êD'@¾àP]¿Ó&(;f3¿æ,u
Ü¿ß|c0"ŠÇ¿Õ?\hØþ×AGNbll?ïîÊKlù"?ia‹}ÛÃ?-m•·ñº?2€+X`»?^½¶oÁ?he¥4ҏ?ïÊôþ‡-z?|ˆúí	?EÜæˆHî?O£áòZÑ%?wÉãëgÙ1?zJ°Ï³/5?ïoY'1?†N‡í_Ú?ƒ^+¿–{ó?qƔګm©?"âþûNŸª?`õTôÜ?ïqŸL}M?†,Ë%P?åì|pÜ?!çì&¿]Ò?'µû˜ƒÙù?†Ó-zÃ3FGL J2321.2-6439@sځ¿½ð'ÀHç( 2:À:ªößÅÍÕÀ<	ø¶_¢þ?Ù+ÿY´H¿@'¨ÀSÓ@4ôBp¿é§ÇQ/?¿çªyW@¿Ùù¼ÚçB¿á>ãAAGNbcu?ïäFK˜?pOGï"?:s¤.Þ©Â?AŽ.©-"l?hk?â%S?n¨þ^¶`(?ï{o8c7Û?ÄË=ˆÀ?`ÑZä`M¦?g3öm<?ŒïÛ.õÊ?ŽÔ¦îNB?BK³|?'z'µŠ…ã?Š¿ìtº©?~k"k#T? up¾?Š³I?ï¸?îòfp5«?'ß7¸ˆy?a;©:OD?gGn´îÚ?Ÿˆ_|ÒÙ?'ò"L‡á3FGL J2321.6+4438@Z¤[0HÀ.»›>µGuÀ:ýþž1À;ºÏ' =¿ÚRqÿn,%@k¢Câ-@ÿYfú¿ç¯3ëáæ¿ì8æv1Æ¿ÛId祿ïÿŽî½AGNfsrq?ïî†A0vÈ?e‹–wB,»?5!}i>Ó¿?AÁãx¸P?]«D¼¸?c¢£D<wû?îõÞ&kK"?£ãôÚý0?€" Ōt?"-¦ÀLT?™2ë/³Õ}? …è‡NA?í«ÙZ~?›ÚÔɹê?ž¶ÛŽH?‹Ç#Þv‡l?¦DvüÎØu?•«Ë"¦;?îḾç¥?›dGg¡¥?g7jÜ×à?i@wü_?©¯ÁM3¸/?šÖkB3FGL J2321.9+2732@Xêãÿï9À?A§¿Í
	À9bCá× 
À;¢d¾£À	/]k!Ð@Hÿnàˆk@BPàW`¿å']竏)¿â's%Ui¿ã˜|+RFÒ¿â	&I{RAGNfsrq?îO5FÕ?«2Àá‡~S?ha1HRU=?hõ—ðÂ_?©†˜ŠŠm?ª³uŠ?T?ï¼Q^††8? 
]@ô?RW5hóÝO?]ÿ~'	–j?}AƒbìÂ?~ò3î.òR?ìډRöŠ?¢8ù2…RÉ? "Ð/ę?RçÚõ˜?°áÍX5ea?›`Í´¹?`6&Ç?‰!¦âºy(>ý÷ìVuÔ??zÑ»?‡Š˜ö€#C?‰*,YŒe3FGL J2321.9+3204@YkìAÝ"À;àÿ‰¸{À8«ˆTüÀ;j´MzV?öØïæ|,@9DQáõ@,n;òÊb¿Ø›£¯¿ä%:cËxÜ¿ä˜1&éxÕ¿é,ÛGÁœAGNfsrq?ïÎʦO
q?yCå¬&JT?aÀ°_Œ"K?fiˌø¢í?ot©Qhû?uλÄOm?ïºl-}Q?}Ij¥?V'oR›;?^J½/ºBš?}@#¢l±'?x[~ì©?ì 0Kò?¨!%FM©Þ?°š–˜°L? '1šáÑ?¬ÉÎ;Q?™ùR§F¤¤?ïÊ9âã#¯?€!òhéy?5ò¬¿|~7?BDéWpÖì?yƒãÂv`_?€%±!›Br3FGL J2322.5+3436@Y·ÃŸý`éÀ8ÇóÀVœÅÀ9þæªÄdHÀ;v zÉʺ?çS¬#xÄÒ@"DvÒoN?÷­ µT?Ñi-竹¿êAb7­–¿ÐE­e¡¿'ãžSbAGNbll?î^:ahš§?­m×ÿ6ˆ?GúUWH4§?SAÁgȤ?©¼p"4½?­V£i–¼É?ï\²¤§rª?›ï¹S^Ql?mKn—ïµ?ƒ—ç£B!?À=˜!¬²?—'ˆ%Z8?í艷…"?˜u!ã+¹?–Y*§?G?‹"Έ´…?¦Jé_4C?'œ;v	D¬?ë®Né÷Ãï?²Ô_oO}õ?aû{7/Ãt?vJ	÷àÚ?ÀþÖkD17?²°¨óøžQ3FGL J2322.9-4917@tè¶@c^ÀOÏ`%ÆÀ9Ïûf=K»À;¨Ø+¥ 8?æD`ؐ'ø@lõÌ ?ÿPý Q¯?ïýÆÖØX5¿à'ÞIvìq¿ß̃ˆ©¿âOuiõ£AAGNbcu?ïs‹"]d=?'±w%q?b±¯¶ŠêÜ?dz^փ€ü?Žp¯;6?«uN;?îô"{é"? Îþ'çP?z¥cû"Âñ?€°'NèÙ?šÄ7ƒìl¦?œ€ÜÃ'ìy?íÅæöqùÑ?›/¿«'H¨?˜6µpvï?…ÜöS€$?§†5à¥å?"@ÿ±³¾?è(ãñwŠ?·'¤‰A€ã?¢>#gÁ@?œ‹ýûòZ?ÊÐ#–IÑ·?¶
"–¡^\3FGL J2323.4+5849@[ïÆÁ#À3€5'À7Á»øi3À:™MüUy?þœlâ×P@
†"Gwã¼?ñ'‹h(ˆ_?ïÿeÛüëy¿Ë¢:§ñ¡¿Øh|U»ô7¿á—"¤%OTHERsnr?¾w‹W¼?½Œ9ÞuU8?äAyk3kd?ÏÅ!"3?Ͼ"Òl¦"?ÌÕ\éä?^ż§hâ?yÁ–)]i~?â½Ý<ûã+?Îׂ<íÐ?ÚeÉw'??ÎéÕTe1?ÏCEصë?±ý€=ßÁ?Ó]h…F©ñ?´©3éËoÕ?ÝôïÌû?¶*¥öíT?¦¿Õö[?m? ËÑÂ.?ᓋš‹+?Æî@­¾Œ?Úï/ÿ¾?ÄÐ~4k¤[3FGL J2323.5-0315@Sr‹`òËÀM@TƒæÀ8,ë-
$FÀ;K_Û1ê^?õðÚmÊ2ê@©8<²bé@}8ßðk¿ßû²WDy¿åÖhãªp¿äƒcþ"T—¿éN,™¢9AGNfsrq?ïß=W?jå.+ÊÖ?R·"¹àæ"?P±0"?g'ùô4o?gÕ5[ESY?ïÇÔáÕd?|ûVýn?H؊ƒ
¡?Ryü†
Í?xú}Ô=X??z'sA¢hq?ît8 0Ô?—æñ9¢®¾?"»v'?‰™dûU"Â?½ê‰ª¾g?T/&úI?ï_•T2%ñ?"³Ñܪ¤L?IN‹ñÛ?P§S»ùè=?"Dû^R?"|É.Èî3FGL J2323.9+4211@Z"º@Ù$À1Îÿ:cÀ8—nVõ°À;&Lké]&?Ñ32á0:@òÏ1+7?þ3'€ù9½¿âVÊÚóñ¿Û6fã}­¿Ü?_|ùa¿Õ¬HßÂÉAGNbll?ïùÀ6ß
5?GHó¸äp?ŒM"Ìâ?ˆ*}!Wf?F­šÑ=§l?FLMOú¶?ï¿ZÊí?}ã4s?U³¬Åÿ×	?W³†Kßÿ9?zæér"'?zÇj<®~?ï:MÏ•Ÿ?"ÿJ9+?~>#ä½?sé=b?'5v–ÔDÒ?¨í÷IÌx?ïY!é¿?"¤¸Á]—?-luš¯u?3	y¥»?"£¢×¨Éü?""årߜÄ3FGL J2324.7-4040@uãV¿Ê…ËÀPå}ßÿ¯xÀ8´@éÕPÀ;
®J*Æ?ë<¶ÅrÍ@
Å6ϟåä?ü*@›P©¿æ•¡%ª	¿Ó~ÉDé$¿ÕN›}ÁÄ¿Ô],bAGNbll?îYF°ir?¨•R^+F´?p­Ù¹n œ?t,1¹Ó$?¨UãmˤÈ?§úD¤?î·§Äô©†?®=¬§JN
?€^¬ú?"øÊï­o? ì¯"r?§7nëpg=?êmêQק‡?ª#"žœ¤³?ªðPŠÇµ4?™Ún–N<ë?¿…+Þé-?¤úZvc·'?ã÷F!}#?½Þ"
ùñî?rsû^y?"e9®µIÛ?×
L}P(?¾J:‹€Ò3FGL J2324.7+0801@VA©¿ìêzÀH†|à%o%À9];÷'À;*Ž:Á¿úÖMI^î£@/Ø;Ù@5æzyC¿ÄT‰ Žfœ¿æ¶à'>祿ÝQ"	ve¿àGBAGNbll?ïõ'#|ë?a‡cM›+€?@ÿM
©
?ŠêÈPp?S)¨ì5M½?a`§]x[v?ïÈæÕóš?x6XŸ-æ?F!¦!?Nc»³·¹™?xÈ`££O@?v_Õà&H—?ï-¥Gƀ€?…™ÊfÌO?~e`¿…ýZ?r«ßLŽÖÅ?'±þ×Np¹?a"9§&?ï®Â"ý*?{ÿ´@™ø|>ëM¡DyG>ûÂfPU•?"H‹Xd~ž?{÷PV…Fh3FGL J2325.2+3957@Z`u>p~À3ûý€É¾ûÀ8ñ?Ãdn?À;^>¢‹±?øž|DŸ[@—ò'OOI?øœcÎ[˜?ÇñÃ.ñã¿àzµäå¿Þ´3ôNF	¿å¾ÄŒó$AGNbll?í¼ir B?¼Ñ®ŸÆ²?u›†4è?‡ØZò\~W?°Âü½ì'?»Û—
ׅl?\Xˆµ?Ž˜.º:íæ?lg7"õˆu?z«Ûºt?†Á[àp¿?‡_>ÀxMÿ?æðFÒjO®?¶±ú…žW?À@<ùíß?©º©P×t¡?Ãþ¨®\Ók?²ÙÖ6\áî?î­"™-¤?›†¾UW€?o¿CI)5¦?qÊsÊú€?£1â;J'q?šÑp9õy^3FGL J2325.3-3557?ý"YßDs¢ÀQmœýç!À8¾¨C€ˆQÀ;‹³ünñ?üÑÞú¡Ç;@­¶Ð·?þ'Ø	kä¿Ö¸§'(¿ãpPJU¿äÉHROX¿ïÿæNËaŠAGNfsrq?î°Ciޒü?«¢[fì?"+ފRØs?ž®³ÕIûÛ?•Ë´9ÚÈ?¤‡:¢aŠÂ?ï"Ò°å1"?«ÀóýIé?yÖG¬‰?¢F,ÂÊ)Ö?•0!îÅ|?ž9™ñ6Œ_?âc
¢?³%gHÝà–?Ó/¬Ë-É?°Ln ˼E?Àrc§?¨¿lâR¿^?î¹zx-~?žŒ\IË%?€âÇ?›À?ƒ¼¾m¼N>? /­Ø–8,?œjëv3FGL J2325.4-4758@tÿ¹ÿÖ•ÀO¡ƒ_›q
À8÷.=*,úÀ;wv¡G
¿ÂÌV|°Í@CDÁ{
@|| 9›Ø¿â®Øê,¿éêï¼TÉ¿àŠj%™í¿Þh¶ª÷eAGNbll?ïñÁ ìù?c7õþ|s?ä¹€4þ?zÙ¶Pœ?Zÿʎ
?bñÇÆ7ÿ"?ï¿+ìmd?'ÞëZÑgd?Gã`›"›Y?N¡¼oeK?}m²VÛ?'ÜNd´†?îÝk‡._(?Œþ©ËñH-?|=}r¡²]?hÅ%%n‰?C/½‹®{?ŠƒYީƨ?ïßtðB,?ÑÂ-±îµ?%e£L"/?)Øv"ʳ$?™F^'…?Ða—M€b3FGL J2325.6+1650@Wɪàú¯ÀD®ö@c^À:02ˆéH.À;ÙÏsëŠ?ҏ‹Ž>Å@ÎÙçè\@Ï\ÿµWe¿×C[Òí*ï¿â.¼Á'ۿߊ‰|§+º¿Ü	¯j«qAGNbll?ïú°.<›?<§ükùÖ?úê‡s†E?Þ¯¾©?Bê^*r?:ž°Ófýô?ï¸8(Ô?|cZÐ.?O¹òáœ5,?S¿ÑÊ®¥°?ì­9Àñ~?zª*uNW?ïR6`L8?'íaÛ¬N·?~\üð6õ?vè½kzñp?ŒP3ï¦VŽ?yÌÓÅ¥?ï…p)'ÚT?'|µºç®?@°EÊ9à?D‹æ˜^‹?˜ñ>¥Ì´?'EIo¨Ì3FGL J2327.7+0941@VÎ]ÿú÷ƒÀGûæ Zé[À8sþk«IÅÀ;Sï«&\?êê+žQ @uiäu5@lÆ 5T¡¿ç',ÐÔªx¿çž¯rô¿/¿ìûXùé¿ÔHæ"¥AGNfsrq?ïü'¼ÌöÐ?=úëˆ|r‹?44úϲ7?;?¼¦²aá?Ø"uç?!{¢ÅŒe?ïÊۂˉö?x›/l ?En»6v1?PJœß	?wäg3jÖ?uúïZ…ér?î¦uí~q?'œ žÌÿô?ˆüÅie?'MØ-+Ëz?ž²ß›¥Ò\?Ž"ññe?ïäÐv2÷D?sºQ˜°>üRÐVÈ?¢ÂëôÚç?jöå—hœ2?s5'C´z3FGL J2328.4-4034@u×TߋrÀQJërªÀ8r2$?ziÀ;M=5´Ã?ï¹+è'#~@Ïz>üë@wö?ŒÝɿݵÓ€ná¿çñ@/׿ã¥'¹ßü¿ç{$Ö³šAGNbcu?ïñõœ™ä?\… u½€ù?1éPq ³»?,´‡ñ{ýZ?Wšsބ?[ó9Qc¯?ïÏBk§?zg2©e5/?C‰8C7?KÍ+œÕ³?vT÷Á˧?x²	ÏÊÑ?î¼)ϳ×?RøL릔?ˆ
ü¥?yñJñ'#?œ;6†—&æ?‡¦›sTæ†?ï®TÝ!$-?ƒÐnš"Ø1?|—î3!?*fW7ÍÏ$?"/χڏ0?ƒ­¨D¶W3FGL J2329.2+3754@Zb'!%¶À6*ÅÑqwÀ9^'åp1ÁÀ;rùÒ¿U¿±Ž7°ñO
@Êt[òo?þÖϟåãõ¿ÚY^ÅLÄ¿æèϼý]¿ÓœÎùÁ¢¿ÉËV=ô?AGNbll?ïáQ4—C?f{˜'°ø?4­BŠâÛ?2E«Z…S¦?ll™#_?eÜ6͑ɰ?ï´Æz'U%?۝B6—¿?VjûÝʺ`?Yr«Õš?€ã±_Ñ?}*Úô}?îÐ^˜¼á?Œœ‹Ó¹Æ?†&OYI?s톆Sñ?šó™À·;€?†*>c5ÿM?îÕèÇ"ž?yDE2¶Î?0)±2`?AÆsíÕÏ?¢!Tañ?ièUð3FGL J2329.3-4955@tÀ@%NÀO(?ßéàÀ6¢áÌ8RWÀ:Ë%Ü2›@Ñ´d ;	@ ft"§lk@…ž†"W‹¿à®•ó­óT¿äâSþô¿æ|ÖJ­€à¿ê(…	¿œAGNfsrq?ÀÉÝ?">~n¡ªÌ?jšMËÐ?q‹Á¥s¤?'Ü8üZÃÖ?'{Ϭ͓¨?ïÓºFMc¯?yԊìUÂ?I*n\€?j'(4Öð‹?s÷‹|=B?tœï®6)?ê¿hҔ©X?­P*?Å%?·Lôø\Ì?¥lViá?²·Ärþ%t?¢]nè÷¿?ïðŠð»Mþ?q×}$«?‡ú¤5Ô?)Ñ֗ìîD?^]Þ¸îàS?qË0*ž3FGL J2329.9-4734@t÷:ÿ°NèÀP_¿î—ùÀ:*Jmâ\À;½êi•ÅÐÀq—:ï•$@Á3¼p@Úf€'ŒŠ¿ãýß-;f¿Ü•AþÓ¿è÷%L¯tç¿Ë™ˆ/lˆAGNfsrq?ïÈÓW@?€˜s8eB?dñdC‰K<?pú´Exÿc?q¢Q5ºG?x»Ð6Ù?ïÓ÷²©[Ï?y‰ûJûF?BƒºùA4,?M'¨ªÊÅ@?s³¯L)ò?wÉ¡†!NW?îtÎ%ŠÄ|?"Zñg©ª?"üÜ{Öë1?…l9óƒÛè?i^ÒЅr?Š¯ìµ‰t´?ïÓeý²ò?q·#ú(C>ÝÆ`—
+8>îûhqV?vEŽ`ý'?q¶Ä¸3FGL J2330.4-3726@vJÓß°Õ ÀQ"ÓÀíÀ:TX¸þ¹¯À;öBzÎÓ7¿à²$'( @*éÓmо@Ž€¢§µ¿ã/Bóçæ¿ã8ßi nÏ¿æȹz¿áÁÁ¯@—AGNbll?ïÃòßB}O?'»A>uƒ—?V¡R+?³?W$)lÅ,.?x^;Óñ"{?ž`厡æ?ïµÛ1d?…Þ²Ճú?RnÝMùe?f`û5rªÚ?€y-‰çÐ?'´Cœm;%?î}.Yœ?Àøƒ>ù?4î¨Úó?}Ó×øú¸à? _âl¯˜?‰#ºaLf?ï8'õßµ)?‰Üñ,‹ÿ?D4šÅ?Fœ…1mÇ#?˜LÀK7µò?‰¥àÅòµÍ3FGL J2330.5+1104@WD¶ŸÏ=ÀÀG†"`LpòÀ9¦5\_VÀ;‹võ)ã(?ÅÚ­Âè¿¿@|û£$ð@p¯Àw~è¿æV< Õ^¿çüŠ I¿é	¶™üã7¿àpý~ÎðœAGNfsrq?ïí…ó!Ž?\묌­Í?FLíbð?E¬­©&)"?Y¬sGt1z?Xs\xù¨?ï•ë›C£?…ÈÕ×K?Ó?XÃj£	f?c$÷	ßVä?‡l«æÍê]?ƒ8"×êÀ?ï Û­"|Š?…PG«	Ë?r@I—>÷?pü¯Õp‰?"ú;
Ÿ*?}àºh¿?î?UvL?šÝCV¯\?fuÑt&ª·?dßíDq+:?­t­¶0?š"$ Re^3FGL J2330.8-2144@FtqŸÀQº ÒH7À8é¦W>À;'<b†ÝÕ?õ" pãÂÞ@±±Bؗ±@(‰‰V*"¿á‹³¾¥¿æ]'O7¿æ,‡JÀ J¿íÔo6"nAGNfsrq?ïÊ£z†ÁÑ??AD©»?kb}TÐt
?€Òâ+ø?iú$mº)?gIß­OÆ?ïÃþ'?~ºz<3ªÐ?M(Tg•E.?X 7DeW?zÌöc'Ž´?{1°¾'[ˆ?íÁ¿çý°þ?œÓ+zz8?¦ë×fz /?–EýšÌÿÉ?™ðT3TŸß?Š£þf•?ï¦lLŒ®I?‰ªT?FNz¸ÃR?PÁµ))?…Çõ(áÌ?ˆÞ©]u(›3FGL J2334.1+0732@VôªŸæºµÀIM]߯' À9P>±·!À;œ‰çÒ¿¿K\¹ƒ2¿@*^%$QÄ@	À¿£C'¿å"«ÂªÎº¿èRk);/¿ëŠwV	L¿°qÀ•9–,AGNfsrq?ïáç?'Ù?mÍ×b¾¬?PÃ*¾«?OëJˆl?f~ƒ¶Ño?ib ªL¦º?ﷄ	
Õ+?‡8¿-t?Naü|Ջ?]3'"%[?€>—œÂç"?"Ì–ñe?ïÉ«´I&?"÷þ{K?/¸¦Ò?n¯ÈH÷jç?"&ˆ}ˆ±"?iT!ýÐ?ïDî]s?'1Ôcí÷=?9*¬›3&'?HϕÓÍ"¦?—WäÒÎ?'%žƒP'3FGL J2334.8+1432@X$՟Ú%{ÀF0•ÿ±%§À8èºÅcLÀ;<
MzÝ?ó
…örc@CÒÏÆ&j?þ
j¬¾d?äh—ë»ò¬¿Üƒm
¢ùÈ¿Û»ì,
þ¿àÈT˜ÉAGNbll?ïõ›*9†?`µáD‡Ã?)Ïfã!)›?2¨ÁåóÙ®?RˆÜÏ(Ά?\]ê$›"?ï¤í!|™ ?"ÚPš¶1?SÙÂÅðß?Zs!¡hÓõ?"I]àٛ?'ïé2?폸np«?Ÿ«µ"d‰ä?žÞ'é×w\?'ÕÝVÛ<Ž?§•7©-9€?˜¤jyìq?í¢Îlhºó?§¨o'§§?js‡)¬(ç?oͶn–?²ðclÇ?§I¸vr¢3FGL J2335.1-0133@U
>?Ö¯¥ÀMGy`>.9À9çÜÓ«
_À;–a(	4?äÔºŠˆ@)\šµ£@°Jߢ<€¿á|8xóÌ¿çlmiÃp¶¿åd*eÈö¿îáõrª¹ÊAGNfsrq?ïVVS"x?‹W(2.ú?jÇԔcšö?m¾Ý¯[B?…8uF{?‡n&ðœ?ï©Ñ±[I?˜Q"6Oê¼?vg÷¦6J?y·ï©:Ê?˜pÇàGx?"â%Áؚ&?‡ÈÊH?"½Ù2Ôg~?•BC?ÊBW?…§¼}QÈ?—ËkÇt˜?‹ÇŒdä˜?ëd?5ÆOº?ª>¡é˜Ë[?•™DAôÃy?ˆeÚiÁñþ?¿wµAPQU?¨c¢*aâ3FGL J2336.5+2356@Ym¢£Y6ÀAê.Íû¡À:SefŒ&À;àø‰éù-¿Ôl£÷ì`;@
"yöf#K@ã_`bÁ¿éD~Lêœõ¿ãKä;m-D¿Ü4H‰()·¿Ô/X×*ÁAGNbcu?ïÃ`ØÀcù?†˜Ž,ˆ[?7QÄV}hC?KÁÇËù?|ÚwZf,¥?†nºº³?ï©;7ftZ?€xҕT;>?Tc«¡———?ZðyAÈlí?ƒ$¼²/öE?}Èk¥Iå?îÛ2¼ûŠn?ŠsÓ7?"Nº÷.6?réÆHÖTe?š,?…dìô	¿?ïdË&¦"|?ƒŠºçg¸?3ü™CY"\?=8hMøË?"¨Æ *[?ƒqND×»3FGL J2336.5-7620@sIÈ MÀCú‹ Z›À9Ü-$%y6À;ΞÚK:'ÀßU®dÎ@é¥J§Ä@¤2`Ov
¿áre¼â
¿åÕï°Hÿñ¿å
1÷Ž¿Ú‰N³A`sAGNbcu?î÷ RO×?¡1›=Eõ&?c_	$?g×Üt†¡-?ž ""æ? ˜Ê	ºV?ïÁjœo/?{¥'2¡bÉ?HR±¦Œˆ?QāÕO?|@n\"—§?y(Ê
=b?í¢2B$ë4? iNĸB?–3«9 ?†"C‰>?ªÃQˆ|­?™›êÚ?b?ï¼"NÒÜJ?}ÕZ§4Ñ>îÉçÝ-¶d>ÿŒåŒc0;?€ï¹ÑQ¡·?}Ñ!73FGL J2336.5-4116@u˜`@|ÇÒÀQG8à^*À95±/¸TpÀ;¬r9€
?óÙ—ïun@Ô÷!'@ê?Ðz¿Ü…¹}(¿á0ýg¹œ¿égÄ^á"6¿ä©ÀkžVAGNfsrq?ïé² }µö?eñ÷.¥?\(ìÉæ>³?`û¦¹P‰/?PqÒ:­×½?RF¨n™g??ïÑ|ƒi?z[à	×7?DvêG^?Pbg'°‹?tå!]Á?w©@Er#¯?ìò7ú=¹§?¢ÂS7—·Ò?ªôš÷®¸?›ÃÀ¤ØÃr?¥çåduåÛ?"%_"'žž?ïÑû¶ž?{&LcŔ'?1`œú}o?A;f·6A?v`x§üÙö?z½A¢WÇç3FGL J2338.1-0229@Uï¤hÀMâ'àÙìÀ8µçïhHÀ;n\Âxµô?à¥ß‰N.@sôI"qâ@÷®XëT¿ãæ!¦² •¿æÙ{ªD¿é"~‡øB¿äíëÅ­ÁAGNfsrq?ïòCGu¥
?fmáV®ÿ?A/Y¾åa?Iº¡'Ò6?RíÙgÖs²?a-ƒnáA?ïĵȯ"Ý?Hçéw£?I]¦& …í?RÚs©Ô?zyfãiT?|õ_{}†g?îðc挋‡?‰‰JœÔ?òXõ@?n?ä'§q?˜úVísîÊ?…ÍÙÎr—?ïÅ'	?—þ8O"?RjÇxW¡i?V£ÍŒDO3?žÀ²Ã™Äê?–Óíû—Õ3FGL J2338.7-7401@sYPà"'ÀE%àdYFÀ9ʝ}SèµÀ;¦¶Iӈ©À@2¯´ì@Mlr¹±?þ4¢ÿžÜ$¿åÛá"ÒVò¿ãkܬ¿â¿Ê[ý!(n´¿ß˜Ëe;˜AGNbcu?ïü¼f¾+×?7ÚÙÔ=ï©>ëqhš*Ý>ñHû\¸x?9A>ÍÌu?7xQ)7Ã?ïÄ¡|.?‡18ß—?D¶Œ#'ýõ?OŒfŽÛ
È?{¤½Ž	a?†©"wR©a?ï'!ZcÈý?u›wå"/?k»®]¼?Yœ3z/f?"":¦¢)?rnm稺—?ïüxŠ¼?Y{`a°>Ùb^Û>E#DbYf?<?ùdm?Y{_Mns3FGL J2339.0+2122@YPyámmÂÀC5ëß·‹À9ãIŠÀ;Àaâs'¿œô
Oûp@ρó_³š@nԀu¿ååª	ºz ¿âÑOS'ç"¿áАDõí¿ØswšÚûþAGNbll?îƒn+}'¨?®KœÑ?TJ	Lly?Rír"÷XÆ?§&Í7Ür?®Rñ½úU?ïJ9{HìÒ?œÛ_aû¹?kùªÈÁšM?€èGG~H?"9›=Ê2l?—kV
ɯ?í˼՞?œË0ߤ¤J?'¨äË֘?€@é£GáÝ?©ïÍYYºÈ?—Õbx¹?î†7Š:¬?œüò(ên?iþà[_y®?püFt*¹4?®7®¦]¥?œR š`¹3FGL J2339.6-0533@TUGÀ'áÀO<OøÃÌÀ8:[Ê+1ÝÀ;MQN§-@M¹2;;•@
‡ûÐñI¯@=I#àYò¿Øú"¯-¿ÖßóÙ^´¿áÇívÝÏK¿ìm¯nJ¾ôPSRPSR?täw9–^?|+ý¾	?îÞIiîØ?­ÑEÓܟ4?žöù\'?«3»ego?ÉF¥'þr?¬«öU‡[?ìLX–…Ö?½
4ºIÝ>?¹jé¢v'´?¹[‰ßŸ>˜?¨"j#cÖK?œRþq³?ëì÷þ?¨Wà¢ç?´]ö'ã?¡I…›:™{?'dÓR_Ö?Š\ÒW~•q?ì°
ªV´(?­å'H2ª?¶&uØƆÀ?ªQÜ¿Ä3FGL J2340.7+8016@]öaՈ@1Ó8€z
ãÀ8Kê¸pvÀ;$'ÅA¾?ìhSbÊòÏ@Q\ÿ_q*?þ¦½žÜy"¿É
BÖ
Û¿àŸ@ŸNÜ©¿Ù-ûȇ»¿àPºAGNbll?ì_Á?†ÊÄ/'+?}x>0§ÆÖ?x'Å
ê(?~®KŸËØk?€"Š±T5?ì…"øæ™?¹>	üT»
?­~©ÖLç?«u+r7,?ª/&¨U•‰?±ã0ÑÔd?í
ïü̺?¡á¢
h?ŸævJ]¶Ê?'ŸKþÀL?®\ÛXü?œRÐ
I?䱅!æ'?ºâ¼öžDN?³{b£>œ÷?«§×Òwh"?Ѿ‹ ?¸ÐVî Õ3FGL J2343.6+1551@YŸ'xÀEü_ !¸À:@µ¥8À;Ô+ç—r?éÿ»ä¬@´êÓ@Q¥ÿÙi"¿ä¶›Þuõ-¿ìårÐ×ôH¿àKcEŸœh¿åm{ 1ίAGNfsrq?ïâ׬R;`?~Ù}œg€"?0ÕkI²Ë?2†v [OK?k
¦D'ˆx?~ƒ·Kêç?ïOyfQwe?•‰êê»×¶?iz3áOœC?wôþøN|?'ጹ§‰?'Vcwö9¸?îDÖ³YÎ?–€ŠÖ†s"?ˆ™£‡%Ú?'€Š@ù;?¤PnaT®?''3>åÍ?íýÞxv?¡û1,¨?Ç?x.2†Úæ?]¦¹ó?­";ԇÄ,?¡ñlvâ3FGL J2343.7+3437@ZÝþD5À:2Þ@'—GÀ:Iá`ÈWÀ;¼—•³[¿Öà"·Â@"†w}åß?üþ –
¿ïÿñ;äT?ïþ ûh%¿Ìi•Zo¸¿Ò·½áÍdøAGNbll?ïü°Ç3!?5nmk<®X?:VW®´¦?Z§ˆ^M?4ë0Ñ-º?3Å_¸ûMì?ï³7+5?'Fö>V?\ЛsÅSÙ?q*ь6ëc?0Cˆ‡#Z?}"GýÄ?ïb)lá4Q?}oj?xŽl_\P<?f 	çÔbn?‹.n˜á?yíî8^[?ïÇæ·íÒ?+Qåם‹?J/%¹û‡¬?NYÚë#›†?xÇlÉ¥ª?€¼P€ŸÝì3FGL J2344.4+0549@W'?ïXÀJ¢‹ Z›À:5¾ aŸÀ;·"ÌÐþ‹?âqš¾ÿüò@"ÕÁ=!Ÿ@‹‹À"§¿ã3Ál;¿®f@q<â¿âÿñÊ)¦º¿ïôV©"ôAGNbcu?í*Yêæ?´h:ñ¶s?¥;ÜtLX"?§c‡çý$Œ?ª}í‰?®\d

X?á'5£ô¿?Î]ԄŒ?цÛ-ä?ÈJi/]Ÿ©?Ȥͧíä?¿Êªv*O?ççZÍS¦&?±}=™Pˆ?Ã[á/'"?¬=Œ»D?º!ÓÉ­?¥J2Ã7D'?àÎ*¬¹j?¿Ò±4mò?Õ<Æ멙Ê?Â{¦'‡J?ÂN}ùæÆ?°bMcGe`3FGL J2345.2-1554@Plžà*w£ÀQ¿_ã•fÀ7>/GìÀ:ŽÞ¢¸&?ýdþ¿¹@ü½å©<¥?þ¹Rý(	^¿Ü±—¾ß5¿âFA¹¾J¿áº™ˆ@›¿æ¾ä½ëoAGNFSRQ?﫞±Ÿ2?rPèaz3?2Ñèrbl?8ñ÷,	?"ÄT L?b"Ly~??(?‹ÈïîŒ]o?DÏÁ;ˆÏj?Oë»Å¦åÓ?|\9úoQË?‹
Á¢ñ?é¬~_*ʛ?®À׬xü?§]O7¦I?˜yS»AÖ?Ãv²µkT>?¬K9.!?ïêþÒ7:Â?qe4:³°b>ÞHWHV;>ýãzÛ¯À€?dò	!š?qaQ‰x­
3FGL J2346.7+0705@Xß֔ÍÀJ/&à>™™À9*NRsj[À;1dÂ!x ¿ðò㯽Gt@ì±Ííß?üu§ALü]?ï]cdÿ¿ææ»"!àG¿Á÷=ëTÚ¿ØKÈ·AGNbcu?ïâ:"ûâÎ?rê0QR{œ?…ë ÄÉ?"u¯Ù>¨œ?lÉ<«$?rÏdg¹a?ï˝Ä*gÚ?yìì⏛?FQ¼a)"?Pþ'›óá?wfëÓ?î?w®'!ÛË?íâjˆ²q?ž&÷¿';?‹Õò¶?"?¯¹¨
?©Ñ'÷Ùߗ?™wr¾cb?í¯ºH‹GX?¥U
ٚo?	þ¥«fZt?a³cC÷Ê?²~íæðX|?¥S~^Λ¤3FGL J2347.0+5142@\8åÏxyÀ#Îã¿ØrÀ87¢ò(§À:éß÷KüX¿ñîéµ:ßÐ@u'Ý7©?ü…2ªÍ¿ØGÏQâJã¿Ù	žkÝÁ¿ÝëØM*øt¿×|ÞÀó®AAGNbll?ïˋ—µ`?x
QjN?.?)æ"à¼i€?,k§€>f~?yjÿ†J?w¯½¥%Š?ïRȪÇ?Ÿ'32Ž>D?aLa°yª¿?obO~ŠŒˆ?"•Z´žÑ½?B'"Ü,?í¨ûH6¡?¡ï±oU?ŒÜíépRô?ƒLËÝ?˜?®9B)? [+™‹?ï`³Üɟ?ŠAB·e?â†OõOB?'":õ?"òXA>ÑY?Š<¹Y?3FGL J2347.9+5436@\ož²gÇÀ"•¿ðExÀ:…gÖ¨î¡À;³0¨LÀ
­óõ"@ÏTБÓR?û»ê^Øþ^?ïÇôЙWw¿Ø$ë"/š¿éqF_®¿°ÿçÆ5¡AGNbcu?ï¬pÊÞ¥w?Š ˆõ¥À?h@ZÑ+¨?nM{ä/2?}§mŠÄ®F?†évéƒ?ÈWl5?µÇÔcú?f•~E6ä?u'ƒ®i?£–5Îk?µ;#Jy=?írÒ	=âz?›"h¦"Ä<?¡mŽÃ-?'³z;2‹o?§µr`"2?'"6Á†Lï?ïÞîF¾%Û?u£d?"+^>ÁdÊaw·>âíâœæúc?p†° ã†?u¢rxeƒò3FGL J2348.0-1630@Pe ÕúÀQøM@$³>À8@¨E.À;ýFèÞ?éûß+k‹@g
[@ŸmŠNοÖò"†ì)¿åG@ÿÞ*}рÕl¿æ—ÊšvAGNfsrq?ïðy8$M7?ggMĔG?$¼ÕpÞÚ?#F',U0?\uõ	IÏ°?g/7‰?ïɎ¦•G·?Õ¹°?E‡m=7?Q\èAm"?x˜i"n}æ?€Ö'ø¦àu?îeê%¡º^?˜¨¦Ç1k?ŠÎwT§Ã?çãƳƒ?¢í¿Ðºv-?•B<'¸±?¢Ã÷?…ž.qÊ×?¤ée5?"Uö¿!‹®?‰ñM|ÇV?…¶•X+3FGL J2348.4-5100@tTŒ_¿ƒ8ÀO¦¿Â"OÀ:AÖ²ÿœ-À;ôäq.A?æxނE®Ð@|+Nbc¢@r?³Ê¿â˜ .wüU¿àØÉEiþ¿è&•GœÄ¿ïÿYsÜ1AGNbcu?ï_±ÅÇ£?"›ä'E–?ú*³M¢?'pVDžñ?qÿGµ"^?t"ˆÏ6"?í××M«›¸?«EìÛ¶¿?'7"2±X?''âêãö?©fúkÃ?¥¥¤ýj¬m?ìÑ»]^M?¤³K¶?²u…ÍØtS? ¹7 
I?¢Ø®y2˜?–(¥"÷?뒭5é$q?ªvùÁ$?°#!Cz??žh77$nÀ?³Xs/sb8?£§Tà'×/3FGL J2350.4-3004@0ð›_lw"ÀS-ŸàÛxÀ9åÀ]RÁnÀ;ÂáåbÅÈ¿ìR@ƒl @ûÓ
ÔoX@¤ã@Ì¿çK˜³{Ô¿Ú·Éφ)i¿åÀ«°ÍÌ¿ÔÃUqÃß
AGNbll?ïôz><úœ?Z÷)~#¹?'µ#e"?&E˜"óÌÅ?Tâž?YûsPHÒn?ïÈ )åz?€.^%Ñ?B©ù¦ùP?KÆS‰!Ì4?yšÈN@ã¢?~Kˆ%.–Å?ïTo$ád?†bÍéӊ?lý^)«Q?së/lí·?‹De‡²ÑD?™ÅÆ_tÃ?﹝¢È:€?wŠU~þ®7?Lª‹
?bA%æX?€K4FÕI?w…ËÂ^[X3FGL J2352.0+1752@Y⮁ˆ*ÜÀE_H *AóÀ9èéuyÿ À;½ŽK‡½Ï?ÕUÌËJ@Á@ —ºœH¡@ô_¸Í<¿ë
õ‰Y…'¿³íÁ±]'¿Ý:O®áK׿çóijMËAGNbll?ï¹`'	#?¡Ûš C?Sÿ'ÂÜæÏ?bjÛ»…S?~OÚJ·B±?¡­߂z;?îàÒÖêÎä?Ÿ¸­…'"û?u}©1Ä-?w*2Jÿí?ž†:Ödòw?2v?îпoà,?'o(Ôûã
?‡ŽÔë"bÕ?zøŽlï¡ó?š §¨ÉL?–®U­q?îB]'ÜT?™Ëí«¾ë£?"Á©Éô®*?|1,*JL?¦­¿´U1?—þŒðš¿3FGL J2353.3-4805@tw7À*ýÛÀP‹Ã¿ÝÑÀ:¯pÂ	û,À<
K³\¹?êgZ v±Ò@
ÕÇèa}É@x x™¿ì#ÞùÂq?ÝV'®àõñ¿Øhæ62õ~¿åÃ{GýxAGNbcu?ïÖ:ÊÞÙ?yŸ¤X4Í?[ŝðˆ??eÁ¶jB?kâ©Óâ?syÏ6…ÿ^?éš
H¥3²?ĕ'¢çÉÒ?¶¯Wµv.&?¶äì­wÞ×?¼€>`4I?¹JÐ!›Á?î=èSì+?ŸÇÀy"/>?—T† #wN?ŒûPÿO|?¤1Þ*¯œ?–só¨Æ?迾1â¦ó?ºÓX:™`?Äqijø۝?¸•ÖjD?±;šù2?¨"®ÈýyV3FGL J2353.6-3037@,*"øÀS8[ÿÛÀ9öøŠ/À;½Ÿ_¬8À
ågù8'@=L|ÛGå@Bm€ac?îþ>Ôüò¿åŽ-'*'N¿á4òX«¿ë@–®Ù¿AGNbll?ïÓ4¥_³?€Ž%Eƒ´?[–W«1®?iŽûn$X@?o/̤?{Àêÿä­í?ï¹p€¬h?‡œGL&²?H.»ö¤Ëd?TgYÅ̗?€ ô{±Î?†Iž,?5I?íì
Žr? ºÓýΖ>?¨Œ4²ãR?—$Ò÷'žs?¦ò|ŒCÆM?•'\¬\?ï%Ÿtˆ?½æGÿ¤x?"­T÷b…m?6¼®©ÊÜ'?›&ÁõB©ö?¹ÃØâiÚ3FGL J2353.7-3911@u'ÒÀa"ÀR>"ßöu=À:š—Ëc@AÀ<Õ,ß@¿î¹Ò@Ö@ƒÊ${à@?[?kд¿çxS¨'Ï¿ÛQ´}¡¿à'-Èä׿ïÿZãÁAGNbcu?îâcødê?¯[ìÓTÿk?˜$³U÷8•?£2êJB?‡›PxTv?¨Lo¾cBÛ?ïZŒ´
d¥?˜ã—O®?iu³¶¥ÜÒ?vlwÁÈYp?'³Þ¯°?•,çH‹^ù?ê6hu?®ÓùEÁ?À?´²ÕlÆ?«T?­mËì"Å—?—ïÂ24­?ïÉÌ3Ï÷?'2¸^ yE?`‰G£É£?i˜ßeF³7?š5¥p'‡í?'L²ª"¥N3FGL J2354.1+4605@\+'ÿÀ/EšÀá@À9øÈHٍ¥À;Ñ*èáÖI?êÏ	\8ÿÀ@‡Á‰LÅV@Õ?qZ
¿ÞÆüE¥¿ä%~‹•¿îíi­÷'¿ïÿŒ"ÅÁ¸AGNfsrq?ì4OÈ;Wn?¹Ï€>iØ?¸FRVà~?·}ã'ƒo?˜\¾×9e?¡!:˗~ò?âän†ŽÐ?Êd"@Ê£?Îä¨à7vÂ?Âeî*±d?'nHø?¾rª=u?éýŽö?p›?­f%t?½¼Ñ·ÚÀÿ?¥¬ë×!F?²V¶–)º*?š"/®!W@?ßÉÙ8U?½ÌcG.Š?Ùl[Ù'܆?Àaù)×&?»*I7¬"?®üùžh3FGL J2355.5+8154@^7†6`å@3@à†7½À9撚Ϡ½À;ÊÛø¹º¡?Ú}'õ2@
áö#l@óðX•m¿épҌÄù¿çä{Óh¥ä¿èëh0"•¿éÃ剠ìäAGNfsrq?¢´œ?§`²¿¨?"÷'>Ч?•$Þö%Q?›VÔ-®þ?¡º©6))t?íR´¦Ic?³&Å'Š¾?©¸G&'?§O߉â_›?¡´TK Ò?¦=j‹?ù?í"÷47ž?¡×fr'×?¡NdÕøæ?ŽiWSo@?¬'u[R?™R¼%?èë'6?±¤gV¦"?À:ð
Ä?«&°Æ
c?¸‰lÄ?©j"¢Uu¡3FGL J2356.0+4037@[íÿ`Ï‰À5ÏÃøÀ9ávÐ@õ"À;ˆô›GõÚ»…Q¹@6û{6D?û+¿K"ä¿Õ¨ ,g´g¿ëvàêfÔ?ÑT'¹ó£ž¿×³δÀAGNbll?ïG­rh»_? bŽh±:?49ëÕ¬?;8¿%°¾õ?–º$Ë9=R? Rߧy?ïÀ;{]O?ˆÅðbpI?S†^¼ï?WyÓÈ€}?zëà ¹©–?‡hRpë?îEKüßSÙ?"¥!'s.?‹"ˆiÖ?zïñŸ‡2•?¤Æ^ÄÁ?'½úWÇ+l?ï…Ž6ïÂ?‰%ùÚÁZ>Î+Š‹hß>å©AV¾?Ž·¹¹›Y?‰ŒdÿÀp3FGL J2357.3-0150@Wb‰ۂrÀNËä€G¸üÀ:h_¿ƒ8.À;çCHT,¨¿»ù´PBýD@³±"
‰F@üªß'!U¿©J·'Ú¼¿èÀ/³ªoˆ¿Ö¯ƒÓV @¿ãk<P,,AGNbll?ïæ–HÈô?h¥ô"4?--›z?2xºP7T?hÿ•{5?gt5%N'?ï™ó</B?Šw~ξ)J?YÏõû?b;WÅü'Ë?†I2Tͼ?‡ÈhÏ» ?>Ç?Fɒ‹èi?ŠQähKUÇ?yÄÓÙ3? `¢ù}
??ŠMÔ±ÿS½?íë9Ó¦C ?6!'U?YО›?\´Úü—é|?°>îçÅâ?šf.3FGL J2357.4-1716@Q¯3+¦ÀR†–ÿöÅÅÀ:~I±ú¹À;¢I
5
(¿ðz)˜Õ¤@I—ö×7_?ü×›£¿åàQ*¸e¿Ø'-˜‹ôã¿Ø,ßÌT¿Õé†lý?˜AGNbll?ïҗDŒ3¯?«s…d?,e c,w?Z¦X©I#P?uÑ4¹kå?ªžl'½ ?ïÁ?ø³:"?'+h¨.Ôd?Dùej¢3Á?LâÉäì!?|ÀÖùo¾?r'P9Ÿ:?ï!k'?…<_4Í?ᴄ0ã?lY¬d·…?"Úî>ÂV?$n-?ïk­ï%u
?†g ë??÷+Mdg?XÜ¯?'¢»·ô?†¥x|3FGL J2357.8-5310@tz WŽ\ÀO~`X/lÀ9*i;,ü¸À;{ªÙ\þ?ñÑv—áނ@g%%ÿ@¤Ï_ÏŠ¿Í@&€ó/¿èh®\Ê0e¿éÛ7¯Õ׿èõI¯»2àAGNfsrq?ïõ"ðŸêÉ?T4^þJ?L"°p<ã?QL)ÇH?;IqŸÉ=$?7·òVFr‰?ï½Ê­]Ü??ßL?Pž5>'»Œ?Vý:Ÿ¬ä†?}HY¬£!?~ÓæÀ2Ѫ?í
/Í9?£a6ßþUÒ?§EÀ¹£Ñ?™Ëú'Lž?§èŽ³Iˆ?˜4"_?î«,J"t÷? ^Ò#–3q?mžÉÑi×?rä0?£}k™ò?ŸãbXG½3FGL J2358.0-4552@tŽ§Ÿì™òÀQàÀ48À:
ÐW›ÈÀ;ñy¥Œ¿÷?ñ²ŠV@3¼ðáª@ïÕ`EK¿æîô´N¬¿ê8IÈuû¿äÎíöŠ'È¿µ"§?۞]AGNfsrq?ïü½,M?96.S²Ê?`!í‡WC?²ú8O®?8nXì§Ö?7ݘíšN?ïÑâsO6?z. ã(Ð?C–Q
ƒÞ?Nÿƒ_ßé?t>ü6´V?xP'Ûj‡?ï^dÏfOq?~"…Ý?t?qÆø³?_Íøhë?Üʈ§z?|,G~ÀN?ïêÊÊóò?cýgÝò">Ä][í^ªõ>Û¬üXÕA?e0µ?cü
ãï3FGL J2358.2-1022@Tæ@.Ä9ÀQDy î?À9ÿ`µL}‡À;ÛQk,žÄ?òYôèõ¢@é÷7"{¥@^ŀ'W³¿åãC;"ÿÒ¿ì7ä7ÍvÁ¿ï´xAk?ç€`'çαAGNfsrq?ïæÉ;ì¦	?iì^çÍ?X M|ƒ±?\ëÏä4»?ZM:ª0ßê?bÝ®Éåm×?ï«BRÕ[æ?š/2+~ïK?W_úÖÌa?w×Ô`¼?'CkïÏz(?–"Egáûã?íF£Ësy¾?£ÀίC£Ž?£ƒ³¾e?šˆ"S1Ó[?¨7Ä¥Ä?˜ZxÒãÞ?ï€OàáË?–Ót:Tá?Wøe}…Un?xM†ÅöõÙ?ŒÿŸXâ£?•Š6åG@Ê3FGL J2358.9+3926@\"aùðÀ6NÚ_\†êÀ:DýòÿfÀ;¯&2™°@À‰£µQ[@½v›<ÜÕ@ªóŸõST¿âDè´¬<¿àÖÙI»h¿ïp J3'
?ì–Î( ÞAGNfsrq?ïäƲ<«?p¢s"H´R?Wæ.
zúð?cŸß[/9?^ŒmzG®Œ?fF®["ü»?ïÑ\£y!?w«~J+³?Oü†k€?W…'µy8L?snî¿ä!É?töq¤Žï?îKÙl\Ä?"',ӁÞR?"úÔ	"?…ß8ÄYy£? Äÿ7<I?ŒŠ$>JÛf?ïû¢3ùãÆ?M	â~÷à>'Ÿø,y>¤<Ïሢ?AvÎqcÆ?M	'Ïx†3FGL J2359.3-3038@)iÄupÅÀS"x $ÎÀ9½¹Ì?TÀ;¶°ê7.¿àêìX@
³¿e=W@,7žÞ¿ç1Ro°ßS¿ÞlŸÖI£7¿áœ¿^­½ñ¿Øê|"îËAGNbll?ï6¤Êý·?©¡¿_··b?T'}
b—?VŸWý×cc?—ô•ÊË?©qSÁ¡³?ï‡KÜ"¹¦?œ`Ô 9žR?SÜþŠ×?\/1KÞ.?‹»
W€;?œÛm"Æù?îÃy?˜<ĀNír?˜'Ìh8±?{2k;vÇ
?¦-¾mû8ã?"-–éõ?î—vBž?˜xÈë¹'?EIÇ£ÜØÛ?J´'-4i?¦9§šb»?˜uõ&'@q3FGL J2359.5-2052@Lù>À//˜ÀS'*ŸæºµÀ:Nè},{‰À;ë?Íui9ÀLEÓÉÁ@»ž6aeö@$6ßæ+¿èûAîs ð¿Þ",æ½å¿áZ˜U²ö¿¤­ca4ŠAGNbll?ïïçÓL^g?ˆ¦¤†Hî&? ¡ä8Âm?'Á‹BE–‰?^à?ùÇ?ˆU>{Ù½á?ïÈú/*Âg?ƒyRê—?BxjZJO?Kr¯¶Ið?y3å}Sƒb?'æls©•?î÷¦s{5ƒ?†Í¾Âÿí?ƒºèêÕ?p0Wöå™?—-½…$DÀ?Ý;û'C?ïÏöєï?v—̺&ä;>Óª<«Â,¡>åiU1EÝ¿?xˆ
˜X?v–àëνg3FGL J0000.1+6545@]lh‡¨ÖM@9Aâù^üÀ9ðÇô À:æåèðð?óÇî@
©ÛÖU@I£@Œb$¿ÜTX
ÇÉ¿æRGÀ*tj¿í$[ÒK+¿ÕÕ¤l†fUNASNone?µ=vzsÄ
?³ÅtaÍ?Ó7EÅSªL?ÉTDõ=ŠÀ?ã¼®N²X?Ë´'^óqÓ?à²E!l;'?Ó7Z%	En?³'[‡?·8C8o?ÙÔkæEÄÜ?Ñ<џz›F?ÜVN{©V?´<©Å\z?Ǎ~½T‡u?ªá Þ!?×âò&Sð?´Bl#Ö<Ã?ÖýÎ,³w?Ái¯cäÒB?ÉßiÏhŠ??ÇyKøÀb?Ü|ìIj?ÃXLMëú>3FGL J0000.2-3738@u–'}keªÀR¼—žÖÜÀ:ÀঞdÚÀ<åS¬O?ÙÌd3ӎ@lþ.ϐ?ýÞ"?pq?Ã}¸X‡¼´?£ß!W tֿԐÞÎX¿ä½÷n®UáUNASNone?ïח§¬?~ˆ¼¼w¸?Q	þ¦ÆÛ?Zh·¸"–M?oâST¡™7?|·"´?ï}£µÓ?Eù[€¢?aª%ë®x?eÌ¦)æ¡?Œ,‰>vß´?Ž.¡>bï?î§7BÜ|
?'ƒ
€÷?Žÿð	Ó)"?ùæý`?›™Ÿ†éá?‹¾›];®(?îë¾Á®>?•géÿ+?tô
M7%Û?r«|²p–˜?K%6ês+?"É|9ºG3FGL J0001.6+3535@[êU!š"{À:0AÿŽÁÀ:iTz«—ÉÀ;Ý+€À…¿þ³LØç@ÒèDÍdw@ÍÞ?eñv¿í"O'…€¿×òp'@ƒö¿äSÿv¿Òw:/aÿUNASNone?ïì|̇Æ?b=—(,Ò?Iî¡'-ï?Pã¾µœ!N?Z^²´þ?]£	G|D»?ï·ððLî‹?ƒ>L&!?Î?Wã±§°Ù?jÖª€î6?~ íÎ5?~³Á`€m?î&ÿק¿?"
áeÖö?"ºíá)\?"Ö9Ü8H?£AiðÕø?Ž'QR2ÿ¨?ïºã3€m€?xЯˆEP?
9ZÂ-~o?€×›¼T?,ùÅ"rœ?wõ3Å‡Œ3FGL J0002.0-6722@sb9-Œ*ÀH‡ê=ö۔À:n»ØˆÂ²À;çŽ
^v?ÔQn:Mâ@¦€®ç	?ÿ#?B‹?·m¸\Nj¿àºj­{^¿Û"Ï2r¿ßÞqƒ±êUNASNone?ïæÞí›o?fÆ·ÞDÄ1?:e]-èû˜?@õlÈyWì?eÔgQ§q¤?dµ×açë?ªÆ?ˆWÄ~•Cù?ZüϧúÐr?a1ñ¾'?‰u{Y{¥!?†Lœý±2?ïîë-q?†‰¦Ès$}?†|ûc=Ñ?wÑlžRÝp?"Äž3?ØÁòì8?î"r¾ä#?"àYNwwd?d+R8mÄ?eóÓeôÀ,?¥všI?"-=¿ò	í3FGL J0003.4+3100@[½³R¨CÀ>¾¾zúr"À:v,­5À;à/Q&cA?ÑGˆ>Rv@
6v5ƒ@nB@p…¿æȼ¦º¿ãVîÆ
ª˜¿ìžr"Šq¿ë÷[DŽ—UNASNone?é>&ÿ˜Ù.?Ämé	šJ?¼qßajÅH?¼†
u1Ð?¹œè¡ÎqD?»÷
Ü4©9?è#1·d´?Å«|f2Ý9?»¬èAè?ºHÝélþ#?Áîâ®Nþ¹?»)=Tmæ?ë–'bé?¦QɏPó?°˜õLk´?˜"«\×Í?³?åÑÐ|ú?|AB?äûÊ=ÞÙQ?»Lç.¯?Êy…|-3Í?ºKv²Î"?Á—QŒWfò?¯7ý®3Ïh3FGL J0003.5+5721@]Š	ÞÀ¥yÞonÀ9ó"#]ÓÀ;…KQ7*9?ã,%2£v@€ÎۚÅê@vç?¿³Š?ïóšÇ'X¿ääëÿd.¿åÌ3Õoˆ¤¿â¾j}£ÊUNASNone?ím{B®‰?²è÷×,¡G? öÜԒi?§>p?Äé§?¨2FøJ?©kFšéî?Û»ý²9#?Ò·'ÌŸ?Äæ	o&«6?Âú§È‰ž?Úw?JºqB?͸-Òr'M?ë·²Imh5?¤oF¥V¾?¨RLŸº¿G?•û&+@94?¶Gd·^°?žE=-Y'F?Þi·–>¢à?À€ÇÕÔ@A?Êp¸^ã´?À©Ö~'¹?Ԑ
'ëE?¿Þ†un3FGL J0004.2+6757@] •þÚf@ùÛ"Ðå`À9&ÀÀ:×t4…BÊ?õÓ.»ª:§@fyHì-@ù…±;!¿—è–¤>/³¿éì¶¥K²¿ålÙ¿pæ¿ëN§.œdiUNASNone?ªnƒb'ˆ>?§ŒI¦Íã?Ùm+Ç:Ÿ?Ï[oˋ?ä?á¢P3ùê-?ÏÝ]üy?ºXë¡é^–?À‹àré:?×¹[$è
'?ʘ‹çAîf?àØ4ùNÎå?ËÞRØçñ?Íö^m(•!?°4‰—O?Øx­\!Ç?´78ÙX?،#Å"¨?µóîËKnB?·I|1ä´?¦ •†Úl?Ýì;¦}ÿÛ?…ïŽ,?ÜLñúu†ø?À‹:€ìc33FGL J0004.2+0843@Yæ^NÜÀJ.ý›¡²À:‰Ù\'HCÀ;Ü=TeF¿ÎJ¬)FÔ@ƒš›ø@gN``=¿è)þ_R16¿Þ'&ˆªÞæ?CC瘿ëÜC·(ºxUNASNone?ïœË»¥ê?Õ½'zñ?r,98½¶?xT9­_Òp?mèõ9Ø?Š29"éóZ?ï]3<ƒÃè?•Ù'->C?f4|‰CôÂ?kkb1 k?'"Þ_Y?"wA|ãÞ?ë~"OB¹ƒ?©^žÂ…;Ï?´ýWŽ9#?£Ýê×n?®#+ï±õ€?œjo^ëô?îÊR:ÍU'?›ÒÄ6o?Pî€û?[ûúˆˆŠ}?¢Ú¶5¶­Š?›š'Þ¢b3FGL J0006.2+0135@Y¡ß¹8›ÀM¥ÿ¼ä!}À:gÇÐ䉂À;åÅÌ'‹_¿üuB¿Ã$@§¡ïÿW@~Å ]®¿ãÙCӔg¿â>$A‡¿ä§³ª*Ð'¿ÙJµïˆUNASNone?ïå CG5Z?rÉήäÀ?:'Žˆ¯?O¢¨'G±{?gšÊøg´ò?o´?ŠƒñE?ïÒnÂÎE?w¡Ç"R?C€µzÚ?MTƒ!ã×?t‡1ú©œN?u˜R2ç?îˆü?F!?'!؝èO?Ž7Mn:û×?}@j?¿E?ŸàyÀù½ô?‹!Eƒ2´?ïÈž§Ñ?tÈÐK"h>òD<鶖?ÄÁªg¡?{ãºóÂýö?tÂHæKù3FGL J0006.6+4618@\ºÚQÎÀ/»µà÷üüÀ:4š"U•^À;µ/ê©¿²¡¿ï‹ìò@èé­@VŒ?"鬿ëªü ¶*¿çùÖŒ
˜¿æ÷/Jàè?ªƒÉ<Ž@UNASNone?ïãöƒ"q?lu˜FŽÕ?X:Ѓõâæ?_;»xq?_Ø)GÅ:Ã?c:Á	*QÒ?ï©âѪ±%?ŠdU"|?]³¨lü4 ?kÁ@s…*?Ðև´0N?…¼ªN(?îÀHa;:Z?ŒC)Á¯M?‰€#Jjô?x¤ID<?›6â3c³D?…†³ËÿŽú?ïwVpއ%?†õF©³?1™ìÄw¡?AW¶2×û?ÎÊ1{?†Údšg™3FGL J0007.4+1742@[<ÝÖàLÀEô™÷LÀ:kå˜u­+À;âƉ¼­¿ÌûÛqïö6@ºS«x¿.@~á`'¡°¿ãøÏE^?¿äl¡¡¥¿åx¨åx&¿Ý@—UUNASNone?ïZLß\E?–Ô
3'׊?Z4š
žpa?\5°=6Â?"sxô?–
ù€	Z'?ï¢Ïjþ&‹?"B«>ä	¯?Tû2##sV?c™K³$B0?"¬¾üîª?\v'x4È?î5
ýt&ã?–…'¾	­?'ÕÖ8̇ï?€eÌ6—t"?£Ä5WMÛ?'n×$Ò?ï3Ÿ´ì#?ˆò!pˆ?L1;[tÕ7?Opl£ë?˜¾B.†Õ?ˆ"72Šò 3FGL J0007.9+4006@\~‰ô
(xÀ6Ø@žUÁÀ:[	Pá™ãÀ;Ï®KØE§¿•Yl‹w¥@Xö§¼@4p yr2¿ÎBœƒj€¿é$íú]Ãn¿Ýn‹ðò›¿âÝ«{]2OUNASNone?ïuV S?›ÈªpïQ¥?Xßz…uҌ?p‹ƒN…Œ?ŽhªüƒÁ?šP1â
à?ï€ï[ã»ç?Ž	òx?ga$¨"D?kªM\ãì?‰ëßÜí½ƒ?ŠzÃWDôÿ?î"…V…ØE?•v\¿¤c?'–7'TvZ?'î:) Úa?¤ŒŽÖx@'?ÜîпrÖ?î®.Ù,YR?"m_$?Xv"½´?Xў®»‡¬?¤Y^LJTò?'¢ÒAõž13FGL J0008.3+1456@ZënÀY!ÀGT<}^ÐpÀ:W´üÀ;Ï÷1$e:?ÜÉr¢éO@PM7–DP@(	_Ð=¿ß¬Ýƒ€Ü¿áqK²0n¿åT†e<ù8¿å£Y
ÄeUNASNone?í½Æ	t?°U¥,4¹	?"®þl,?šÉŒÀ»Ç?ªLà܈?«TÉĎ?íª…ÊQ	?³ÓgE–?—J=EËT=?ÅÏ·ÝNC?±h€:¢ª?­ÁâSã6?춮ò…º?¢Eޘ½<?¤_MW/rj?•T²§@?°ƒÜÔú?—ßI ð0?éH0"?¯3¦øÜÚa?¯Võ" A?¡ªƒK|Ô?Ã̀bÕÞ?ª»\‡¸3FGL J0010.5-1425@UbMÒñªÀR‡&k¤"ÉÀ:"¢ïƒ°úÀ;þŸ¹™ê?ðÃ?ó`	€@#v4åç@w_»ýG?ï÷"ÁÄO¿åä6j—šÞ¿èŠ(‰¥Ên¿ïÿ†S>ÁUNASNone?îô$$¥è?ª=¦â÷˜?¥§a‹a˜?©]¼cÂr?n® N¤
š?wiWÉ\*m?ênvØ㞀?ÃýS†N]¾?±ð¶ äU>?´ü²±º?º›"þ¶¿?ºs"Nj$o?çi0=d½?³Ä"à /?ǃ5'žKÊ?°9¹5˜	?µ°ñ¢º? þañàT?ãÁþvôf?ÁÕrÄÕ_b?Ì­¬È¬?¼Œm FÒ?ÄLèwe»?¸Uf¿W·3FGL J0014.3-0455@XåÄØì–ÀP†"&þrÀ9ÁÉ@PR(À;råB˜I?¯ZP ²Z¹@÷ä÷»ãÆ@MŽÆ,¿ãVaHæ¿êx.ÉRU¿àhà1®y¿ça6+¾¨OUNASNone?ïÆÕg^?–f_©H?8³úʲq–?7x}s=ê§?‹ªÏä"å?–;wX)[ù?ï©ð' ¡?…´'èàñä?U§ã§Õx¢?a!aöý?ƒG(œ?ƒYµf)%$?î7˜žµ'K?–p^Ä÷+?‰"ø9ª{.?w×W"´É?¦!x=<ˆ?'ôPq°?쉊Íeú´?¢O2P"?`!uå5‹"?\ì]ŸTÝæ?»2å¦~?¢6(Âñ`­3FGL J0016.5+1713@[ÉÐúX÷ÀFlÖÓõ¶À:n‹†±_‰À;ß-(W7?ê	UŽIPÎ@¾¨×Ð@D`Þ<¿âŒ]`â¿ä¸—G¿íDŽ $ô½¿Õ°æØÍ®UNASNone?ï»$ë?›;HÃ@CK?}éú¨=¬Ò?"ÑÕp-èÐ?IÓâ¦f?— ¡IÒ?ïdÿÀ_89?˜Ââã‰X‰?g‹Šqæ?yv¦±(°?ö'§ª…?"'Ý$:ª?íãÒ-2s?™iêfçÌ?™YŸwYmå?Š/Ud©Ç?¥!£!€!ä?'òè}÷4?î	hSԆ'?£ŠT*1?ŒtïM«X|?"âÞêÂë?¨L>ïLÀÃ? ™%K¾]—3FGL J0017.1+1445@[«úëÄ	ÀG¥‰›õ"lÀ:"ùdoÀ;Ô_rV_?ĬÌɔ*'@³0ÅŜ'?þ àÀt¤Ã?ïûÛµÔ¹¿Ú›j"ÍNA¿èÇú¼#\?¦´+]UNASNone?ï¿öþh¨?"B²'—`4?c–°Øt!¯?i+sœŒ\?v9(_Ä;?'—à½xu4?懲¿â›E?…¸wì¦ß?Sˆ8,¼{?fB૙<ì?'ì	ÁŸ†?'x0þûÇ©?ííÊßn-?˜2Ç£2?°¼º?+ðڒþn?¢ ‡ }¾Ù?Œ'ìƒÚ0¶?î5B`ÛÆ}?¥íÝù«ªi?p5Â~pÊ¡?}|Þ«2l?ª¥!¢u~Ö?¥^Èïòî3FGL J0020.9+0323@[ªà"ÀMLæ¯ÌáÆÀ:Š£×
=qÀ;º™?׆d?Û±±=¥'@ù˳G@?ú=	þ±vZ¿ïöjÌ;?ïüÃ'I¿É§Õ"Öó¿Þx&ŸH|"UNASNone?ïüöÙPМ?7¤'Î0y]?R–šiá??Õ4ä-¯?3tÒશ?6V~C9c?ï©8G>9)?Ï²V況?^>°^ZyX?ƒ?Üœ?ê$¦fÄ?"³›Lõ'?ïZÓÀ¹?¦ES-ø<?}s­î8¨?tS5Q?ŠÂ†#ص]?zH•ŒšeÉ?ïˆN	·Û?ó&uM>?f
‰*Ë+?hÒd]O­Å?ˆiGVz?Œfƒcs½ç3FGL J0022.7+4651@]uõ׈²À/xpCßÀ:4Õh-À;ºÊá:B¿úŸ/¸ªUÿ@
"€`7£/@F/ßÁœ¿ë"Øz³ƒ¿â"ß½Y+.¿çŃþZl¿ïÿî¼zˆ÷UNASNone?úÎÑ?·îI‡¤L%?"
¦Ê§¿?¡KÅ\‡/?™ý÷5þfã?³;×WÚ?ï²ü[A²?¦»À :?lj:Õ?ã®>Ã0?•÷¾&ö?¡
ñáÍ*?ê¹<špEÉ?¨"·cÎÄê?´Â¿›ãÑ?ŸÆz–ùÌT?µs['uíá?¡sýèíê™?îVU߸b?¡k§'+S¬?v€b>úÁF?…Ù AÔîò?§Ê•ÆÕ!¼?Ÿ9‡'c
3FGL J0026.2-4812@s¥í»YÝÂÀQ°J¶¸À:[7 '½´À<
Õ«˜ ¿Ù-jôb	'@ŠBÅøG@ù1~'¿Ú/õ¾*¿ÝOõd}¿äï7+ª¿á{Æ!ü™UNASNone?ïìl¹q±‡?gäÙÐúI^?RC‡ã;?^ÖW99~R?Tãu"¹Ýz?ZºÞë4ºî?ï¿?žšO—?€6ÅSt¥?LÄ/E3ž?ULE6 ?|Ç®ÌïŽF?}½g('ô´?î‹ÇõT?'Rj¶b0K?•)¢üù›?ˆ>q¨ïß?™r™*ä[ê?ƒ'·­‡<M?ïqçÕ±Ø?†-—1³¿?D» ªi4á?F¿Ïß(Xl?',Dq¦m?…Õé+^õ#3FGL J0031.2-2320@Qà% …²ÀUŸS À:§H>]À<
àO`d?âêñ3ša@;7äs@ç`Kð?¬ûÕ¿ÜSÜÉ͜‰¿â—=x¨Õ™¿ïøô
Œ
HUNASNone?í/‹‰6?¶U¡s!?©ãõàbô
?±ÖáF?š—.MÈñ+?ª"Š¹=ü?Þ,š0>P?ÒÀ¸¡+TA?Ñâ'ô2N'?Ëã܇èO?ÏáÅ·F=?ˍÕ×+?èr1ށü?°_ŸÐqj*?‹ á}?«3À0=Q?·T4éÊ-!?£zpð~Þø?ßs	ËXx?×±s¬?Ót<1Ž\×?Ãþ¥øœ?Ê1t2V)?¹z85æ¡23FGL J0031.6+0938@\¶ñ€
|ÀJtîõÀ:.´iÿxÀ;»²åšùì¿ßçQu
›@
ãtÈG@Aë>":¿á‰Ñ¤fÀî¿ì€|Má¿â
N×æ¿ÄÃ9TyBÑUNASNone?ï¼+™¶
?†ÊNË16"?/«¦7€ñð?7‡3ë?€vk4yÏ?†~Ò	­¼?ïvM¼‰d?žàÿ5IXU?f`c…€õs?€úqnë©U?ŒÔx½i?˜šFqÂ܏?íƒÞ+¸,?™p%NŽ?'|<³3ø?€èNbm)?®ƒþô¼ãI?–~'=õÚ?íäip'Ãñ?£v-eŠ-?IÛ«áS?WD|»ûà,?°ªŒQ²ˆ¸?£f5,=T3FGL J0032.3-5522@sI輜$ÀNÆ6!úü‹À98ҙ•gÜÀ;ÆNóƒû?ÔVÆÚ´/â@ñ=ÐE'@2YÀe¶=¿×†Pn¿åÀ_±krj¿åþ.æ꨿ãú¹˜xÃqUNASNone?ïøŠ4'b?`ù¡úxF‹?'gÅÿ']??ƒ'ÒM"Î?Gýñ궎†?[Â-ÿ±±?ï×<×?v*2k5»?AáR†ì¾?LCèœv®?r2j-Ë?tÜÛ*??îêôý±Á?ŠœnrÑ©?ˆ¨oŽÂ´?|èÖçÅî?–M(Üâfœ?ƒ1ë&'T?ïú{HnÕq?QiВ'>Æ?%_h>Û
,°¾Åê?EüÝ
1?Q
ÑW¨¥3FGL J0032.5+3912@]¼ãÿï9À7ƒIàâiÀ:L‡È¶½—À;ظÙÐÁN¿ØûÒ4{îÊ@|ž©£ÒØ@'â?û˜'¿í–W£]›¿ä®Ús~|Þ¿à¹ýЃn=¿àFÊڐŸUNASNone?ïëò±.Κ?ië´¾{š§?<´®Ùø†?BÏCŠ?`{X;V'K?g£mlœå"?ïQÉ
ÃåÍ?ž†R)Žèž?rH…dê	3?ƒµD¦±?'4½NHÄ?˜™®­ðï?î/ôájM¾?"'A<87K?ŽC!ºââ6?x˜"èTëÌ?¥oéz¢k?ctloÈ?îàzûWÅ?'¯¤76Å?XVЏìBš?ZªBÕÂ\õ?¡5™Æa ?'¾'ô
-Y3FGL J0048.1-6343@rø‡~äâmÀJ²D¿L±‰À:G./¾3­À;þö ƒ-G?óeø¸
"'@šUéŸì@Þ Z¾h?ïú$ƒíàÄ¿Ü®x¨‹ò¿âÓ2þ§L¿ê‡'éô'UNASNone?æ"Äå@—"?ÇÊK—*ZÍ?ÐxÏ"ø0«?Dž̺>Ùì?£í8"5^? ±Œ¸cœÔ?êÐû °?Á!ÏLÁå?³Í
Ç!ïg?´¿>"u?»B^±?µ\5ã«?é?ÝæÔv…ú=?¼ÑĪÒ&?Ús­þ$?ºÝ3èΈ"?¾˜]«0?¤Ÿhšš{"?å!ªv¬u?¿$E™é ?˧[q^aý?·¼gBçd?¿¥KɍØc?³uý"öö/3FGL J0049.0+4224@^'Ó"wÀ4tÙù9üÀ:mã؂µÀ;Ò?R%f¿Þo£78a¬@""^žñÈ?ü>ñŸêìs?ãˆ)ºc"£¿çÏÅ^)½$¿Ë÷W<쉿ÒIûÒ·ëUNASNone?ïâ·Ð?Ґ?yFe2`?2ǍöT>?BBÖ¥å†?jï>bír?x¦\e;>Á?ï¥ÎþûúŠ?†Îœ˜¼[?`%*l¯'?k»´7È¡g?''ùöf1‰?"¶÷²ÃQ?î´H¡½j?Œý¸¨?‡ùš9YƒH?x9£Òx§ñ?z±[é?‡6¥v½?îßKã"›?•גi?1¨'ä?>JÉJn'Û?¡é2}pîR?•
ÒØÿZÝ3FGL J0051.6+6445@^¼âCV–æ?þ3:ß¿À9†'•ùÀ;&±¥ÿÙj¿ÇùlŸÝÍÈ@MB¨ñü1@;ê€fí ¿âÃÔe>ëp¿â u¡<¿å®ò)伿ç:ӓÃõ@UNASNone?æfƒÂ½¤R?È]ä»ïš•?µU¹w'EÝ?¶ï²PBÌ?Ë»9@KÌ?Å°•_¢Á?àv0"s?Ó¨|ƒ~?¦g4|Ë==?¯CLµæÉ?ÜEÿ!±V?Ó¢8 üo?éå&
sU]?¬CbWÒ¯ª?®†{ãˤ?˜ÔµÀÊ?ÀÉÈÑm·¢?¦,½mia?èÓzŽ=˜Ñ?°'WR@7ž?'¸ÃAÇ?…ÙB¥Å¶?ʎ¾®¡yd?°"|PÅx3FGL J0102.1+4458@_;6;%pÀ1ÛÇæ³þ À:‰–Ob=ãÀ;å¡ÔÑ~¿ðV+57ð1@
§òz†Xõ@í@Š´¤¿çíô¬²•¿ìÈÒÊÆ@?ʈJ´%®]¿é®þn–œËUNASNone?ïzU»¶,7?›Ç¥vó?OHµ^%co?Rȁ..Ä´?v¼'›Ü?›cÊp<Ð?ï¤IU–Ù?ˆ×ǀJ?_ûZ'bVo?d*Øj¸ÿz?'ýÂXMÿ?†NFÌ$?íµxHÕ]?šU:"Æ?–Fà6n³V?†‡Ë[Íç?©…\«P‡?"ƒ¢ížG×?ïg/,Œ`?d™.êR?Ÿ*ÚUì?$D<ü"ö$?"õß(ÑO?ŒúŒa÷±r3FGL J0102.1+0943@_Õ*¾ðk8ÀJ†«Oœ À9üÙ~‹÷À;¶Jt˜XQ¿çef#þë@
ÚŸƒéY@…*ÿ²þ¿ÓU3À™/3¿æ)"Á¿à<q—5Õê¿Ó14iØЀUNASNone?ïO‰f |¼?£|ןÐ?B±D­¤Bé?HcE¨‹z÷?•yIƒFX?£=ïs•ê?ï¾)† (?}W±Þqdú?L։fö?S¹Å"Ü?}h7kƒ
?zö͕A¾ö?îmÍÁ"
^?'":u?ŽÚQG	?{Íæ(áW·?¡l"mgÈ?Œ(Ðÿ€ÉX?p?
µ"¢î?&Õ¾@~É?1C}­ix?Ÿ=°Q?ŽümS»Ã3FGL J0112.9-7506@rÑ.Hè§ÀDøûüe@ÌÀ:o5·qñµÀ;ùRÈ#ð À°§ø¬út@
m…6‹,n@`ŸõÔ-¿çÅùÛ	¿æZÅkY•H¿áªú_à˜å¿ÙúÛö,äÝUNASNone?ï¿Î1AH?¥faQBÛ?S:_eúœÑ? ,4*+$?{JO¥à´Ü?œB‡ufÛÿ?ïÅìïl|'?z¬Í;*Ë6?G!Gz"
Ç?Q˜»œH?z%_ZoU ?xœÈÇÍ¢?î¡Oª~?Ž=[Cí¿?…ÿJt¡X?qÇmw-v? k5Q°oÍ?‰¦B³Î
S?ïå¨`¼B)?l:"¿Ì>».÷ý´‡>ÒôÙ@õ?jT<]ÞØ^?lhú‹Åû3FGL J0114.8+1917@`P§æšÔÀE¯ž¾œˆÀ:•k/ùÂÏÀ;âCæߝŠ¿âlä{%vm@
1_C1ƒ@{] :¿ëḯéÅg¿Ï·zn¿ä)nDÅñ€¿â¿#ì:È UNASNone?ï¹Ò
¨—M?žœûäID?`5ö'çê?x®—UiÚè?zûýã,å´?™[¯¾?fIð²?‹¾øñ"$Z?^'!׃Í\?pY<ÕDý6?ˆÕ'2"Y°?†°ö
g´(?îl§"‹?•£°¸ƒ½?•˟`?"ìÑâ <?£×seÿ'V?6Äí¸$?ï/õXª±?ˆ|rAυ¸?ZhÑ#ý$Z?V¥`êök¾?˜Z¿Bª×Š?‡íPñMÒ3FGL J0116.8+6913@_L³åu:?@ߑæFñVÀ9xÓ³pÛ4À;04	t?ä§ÉJaM"@eQ5|¹@ à_Ñ¢¿æ` ÇJ×À¿ì°Ê!:§
¿è‹êפ¿ïýôf]›ÖUNASNone?îo³}ñ³—?¥óíF9#?ŠšžÆ~?'Vh¤v€?¢^ oE??¢¨Å'+ŒW?àµõ£›òð?Ì&Sw	,\?¸,mÌπæ?²¹Ï–}ª?؈ùE"9ç?ÊU Y"º?éø'bVí
?­ó•Š
n?µue'? Å¦!†?ºÆUØも?£ÚÊæ=ä?á-âìôx9?µÂøŽê2e?ÄW†ÿ¢-?¯ÖÍ<ýò®?Óxv¦Eøÿ?µ2Z»Qg=3FGL J0127.4+5433@`3:}ªÀËDå^³À9êÁþ<±aÀ;t»ÑÒÆ¿ä<™$˜'@·ºt°@B‹ÿÓ	}¿ç]Ñ`¥•¿äÔºLA¢¿í–úNÔé?Ç z^ò\UNASNone?í]CÇ?¶zjÌ?™À70l1? "Iàݾ?­K³{˜lò?³·¸¹ÐVÅ?î?AžuæA?³ï‡¶ÖæE?R²DãtÛ?"äìà՛A?¨!Ð-^?°SÁèl?ì¨b(ò?¡È îç/:? 
°EëC?Šô˜¬ÆL?²ºdÌØÂÊ?áˆI.â?îֆ	f~?œ'_æýÛ?H´.Ó>?\ìwnØU›?¢4ÏPßïó?œ}Ì8s3FGL J0127.5+5634@_û
å6PÀÏbùÊ[ÙÀ9†}™ˆÒ¢À;V¶7_Þ¿ñîJ 	¶@åtìf;@°ª_d"¿á>ûù`(µ¿ì•
5üó¿åPS«‰í:¿ÊÑPŸGƒUNASNone?ï-joTé?—ÿiE€?sÀ©¨³·Ã?x/ö•f]?•o(GètÎ?•×(Ú(…þ?*žcî?ªRMžLÎy?o›z,
8?~Ðiý ïÕ?¢¥³YQ?§æÀÐ#XÊ?ìþí-É}? ––pëQè?™' H²Ý?ˆ*Ît²ÃÃ?±¾®ªÏ?›Û|#H?ï6/š5‰'?·Œ×ç?,Ñ?㹶§µ ?™(JÓC?q}6X<3FGL J0127.6+4851@`!¸'ú
À+(iƒQX¸À:ÞC핚À;¬RLÓî)¿üˆà¡bç@Ñy[á}3@•Û_⓳¿á¨Æ0o›¿æ«2œ›'Ô¿äH-û)Æ<¿è‡S@]¾UNASNone?ïòÚ÷ʞß?[Q‹½@ï?6´±.*·?:êcÀår?TÉ£>v¸'?Xa$E'?ᅱnâ<w?Äé}½óÄ?T9,³@§¢?[BçY"·?{&}b›?€îþwL±?ïÖ¤*t?†"SÇK?Ëž†Ïq?sc¯ä/t?•\7IƟ?'´°j{+?ﯸ¡§o?|öyÕH1?$û=¤?̒h?ƒñŸå!o?|ÑZ3FGL J0132.1-5340@rÀˆPœÀO4MUhÇÀ:‰š8ûÊÀ<¨Å†‡n¿áEÉ_ÒE@k~K4†Å@Ž#"ÅÊ¿†Ÿ
[sz=¿æjÉÍhþò¿æƒþ8ø¿á}ØÚ"UNASNone?ﴆDq?¡‰¢"á–?qå"ær§‡?¡L•Ë±ŸÂ?s×`÷T՘?ynS
uÜ?ïô¶&ü?ŽV{\¥õí?\¡±Ñæq…?q…ƒÈé=?"îØ9r£?ˆtfV9C?ízØ/JZ?š:¹Y\M?ž{ÔA´É=?ŽÇ¡¾è?©'î0õÄ?'ñŽ'm$G?î_³wWÓ?رáúp?`Û#mf‹ž?aucÃ/ž?©B'´?œ‰¤+½Ü3FGL J0133.2-4737@q¿'»/ìÀPü_oÒ À:/Ùâ_À<Ê~=ó¿üšg<z.Å@@âH_@¨è?Äæú¿çÇoE»©—¿æ¢Ißô¿ìä
‡Z°?¸K{Íð}UNASNone?ïìÓQŽ?A0 µåŠ?W§N:Œ©m?4ÿN¼©?Mdt®iÝ?QÖûrÐ?ïÉÀ0­?ƒgÍ+¦µ?J>MKU°?dùdÍ4¼?x,VJ}b?¯è·ÞÁ?íô5Mµ³?•8kA
?"RÄÕª}?ƒ.òÿœ?¦"H½fE?'lºÌÕÆk?ïÃÍXzÏ?}½XK
>ûé!%V¢m?œC"àÎÅ?}ýj¡s)s?}·ª¬vlU3FGL J0133.3+5930@`pyåŸ,Àg±j4À:
ˆß72œÀ;i)¾?kP¿áÞÜ°UÙâ@f
uú®@±?ÿÊP¿Î¹¸|*?¿è9@ÔB¿ÓÌ8+¯J¿êwÎkûCUNASNone?é!eý"Û?ƏÅ/óâê?š
舦ÚJ?Ÿ{:?4øb?ȞVôÕM?Ŋrښã4?æéR{ÖP?Ñ×ÔQkF²? Ãùÿg ?©Ù=¬¸C,?ѱ®$fm?Нà<ce?ꂌ¯?«n'ÈÈ,2?±xÊ!†h…?œZÄS¨Q‹?ºrÐeÑ7G?¤=E¨ãÿ!?ì±£éþÏ?¦t=3ñ›?_ åýÞ3¨?`'*'fÙE?¹ô]˜´?¦L¹šãµè3FGL J0138.5-4612@q<w¯dÀQ0Ý)4­À:W'hr°!À;õo|ž¿â
Ô1£™«@
ŒŠâq¥@|äpùg¿Ó1{©Ñٿᇜ|
9¿áT¯baR¿â¹'£¹¶£UNASNone?ï…tUwÇÚ? µäû+uF?Q±>9,D-?[7w»+¿"?ŒlÂÚè'? y,e³f?ï‰<
'q
?"&Rcµ0¯?\þ-¸QL?iÍ7FŒµ0?Š6þŒ³s?'tøÃ[!?î]VÚáËî?'ŠK¶Ê3D?"4h<nо?ƒ$S¥ªAX? ^3«Ø´?ˆt".ð[?îÒñ'¿Í?–>J-†h?R÷¹V©´?Rænø'T?¥ŽI)	Mò?–4܌š3FGL J0149.6+4846@`—*0U2aÀ)ûԌ´®ÉÀ:K8ãv\À;œ˜È¹AÖ¿‹#ÔÛX@šq¾3Vï@õ `]7é¿ê±®B•s<¿éªŸlRŸÆ¿×K4Õ'lß¿ãŠò¯+ôUNASNone	?ïíPëÖ¢V?pä÷´±?'Ž>î¼$-?/+;"e"-?a60:qæð?pW3BBÂ?î[J: 3-?´wmp?"ås–(®?'K1YÓÊ|?¥ÿxrÅH?±U»w®»?î&î²Hî'?•Ymîñ?‹«"hr¿?wŸü•+n?¦¦0M@Ò?'Ag\ó¦?í`Ü»_O?¢j³£ÀÎj?ks‡ÈKå_?o(:,g;ü?´#œÛâ¦]?¢&Xtæ3FGL J0154.1+4642@`¿rSÍÝÀ-£Íi8À:DPXÝèÀ;¹—×øyú¿ñîW@َý@
Ð1Ü@j›`n)Ô¿çLܺß0¿â€w€ƒâ½¿ïÿËeªºå?ïýø£ë,3UNASNone?ï¥,móÍ?AÍ&Hþ?l²Á$Åy?vÓb†;Ëo?^oÐs·7?Š‹P<p41?ï·M`Ë%?ŒùRæ«?ZŒIÅ?tЉµ¿ÈE?}҈͇ü¶?†8(ûÿ" ?ík§ÌKä^?(·?›`Êõ'Nü?‰lªÏR4?«•À€' ?—7†ú*Z?ïâxu¯¹=?tXyøl%>ø3Ó 4g?ܵ:Qr?mW$* '¨?tTQÉt"13FGL J0156.5-2423@i¿m	Ö¶ÀRÆÍÈuO7À:žr©jÇõÀ;äçW'Ž
?ÇÛ_¦r‰Ï@;-Ö'•?þ7>ÀZ#?à);Þ'"¿Û0š5ò¿â°¡$Ÿ¾ï¿ØdÖ°LUNASNone?ïݙBû?o"QÈDõ&?@fɕ;ˆÐ?Bgá<©¬5?nM3X©"á?m•.Ð?ï²ì7$Á?†›rG1?P/VÙµ'o?`9¦=ÑEÂ??b?"2÷C–ûá?î¤5ڀ?ŒÐEiu×Ò?'Ähª/È?€Ù[ž24?šæšº€-?ƒˆÂ€zÝõ?‰^å5?—¨þàƶ?_PÎqt€s?c'ò:Ù`8?¥» ö†£?—×ê•UÔ3FGL J0158.6+0102@cpcŠ	ÀLÁ¯ ê[SÀ:1únƇÀ;Å;"ë½S?Ö¨j²@P
;§Ëá@wÑ߆7è¿ç2rÓ~¿íëMƲV¿1š°.¬G¿Ò'¹'Õ§‰UNASNone?ïèîi¤Xð?p`ñ2?QGó*Ó?9Kž#à?fw?oÎdiXt?WС?ƒÖqP2ì®?OÙJ]}J?_ÅU¦š@?}¨ôëÿŽ˜?ƒpÀM—ü?î|ôì"P?'ÆTrOý¶?…ˆñƒ?såGbiên?¢éŽúwº!?SˆÄ#½?îêª÷µÁg?šøEU¬›Ê?7jÛôY­?P‹"º ±7?¡'M®ì×?šÞ¶ÓŠ	"3FGL J0200.3-4108@p`ì"h	ÕÀQ…=ÈK^À:o×½Á—À;됝T9¿åþi0O@Å2í<™?þüÀZxœ¿ï¤Ew¶ùY?êv–§Ì¸*¿ÞaË.žW¿ã𝫐ÖÁUNASNone?ïÁ¯ï1?£
$ÄIÞõ?IOPÈéñV?nq(X^?|Q¾`ë)‰?¡[8wxÖ?ï"%aÿø¿?'Tù…3ߐ?b5.$Vh-?ƒÙfgA—§?†i[öì6?Š®‹Ì+u?î÷+"ØÝ?‹_™¦ô@Š?ƒº¡¢ˆP?rì£>r³ø?—Ž¾l" 8?†ÍŸ',¢<?ï-ê]}?ŠB"#&?hR£s˜?s€=bL?†܋ÚÙÂ?†ù"S˲3FGL J0203.6+1148@b°r\=îxÀG§>›A:À9̚`hödÀ;lQÕµ©›¿v¸ŠF|¨}@üçá¦#@·SàQäÏ¿å]Y¸`·®¿êÝÍç½g¿êÙ0\áyÏ?Лü,XEUNASNone?ï¾q?¤Žà]â?moÐ.Zg'?t¡îØ?œBt¥?£¼}®–1?ïqÂÿÍñ1?¡"F&
?fô™ ÚÈs?ƒ$+p>p?ÒÄMh?œƒCÏ?ìI–-šÄ¸?¥ÍTaFc?òØ´A c?‹ðÅÃw?¶6˜f'?¢˜®M&ŽK?íXSÍä	ã?°#¼"Ô(©?^…˜ór9?sCVô5?´ÅSz{ã?°	ã:†ÚQ3FGL J0211.0+1922@brVWûi˜ÀCÓ<ŽXÀ:%S'^²À;²V´A»Œ?ÀV
1tu@
µ4¢žûÙ@•€r+¿à`3$ª¿éN·ñH'%¿âoÛ
 ¿ïÿH¯
2ùUNASNone?îÕEΈ³?¯@¤÷Yb?^ZåCç2?p$†Õ3K?¡»@Ue˜?­õ ×KïÙ?ëÂm¶9å?¹0i4ùmù?£7;ý®Ý?¤­h»­Uç?¸PùþÙm?³ÚÉ:?ë›öS€É?£éû@î¶É?®"¢9-&ñ?—3;¦C&?´üGiFI?ñ¼"¡?èB;=`ê?²Š)S/ä?¦Š=ãŽÈ?¸…zV¢²?ÉTƒ'·sã?±;7ïkî3FGL J0216.0+0300@d
\|ؘ³ÀJÌ~bÜn+À:§.~˜ŒSÀ;äȁäq.¿êàB&"èÌ@
!Í°!›@2@·¿êVbÉ_J¿à(³éãQ¿Ø2|mӇ¿ã7µeó UNASNone?ïø9nñ[!?`ó^À!?3
ý½!?ÿæ/ؖ?Lsà˜Óɛ?`]eªõH|?Ž?Ë?ˆ?ã^NÑ?Uè}9¸µ?a[ÕaßJ´?…YÐu9
Ñ?…º#Cn­¼?îö»'¤Fº?‡gEüÕLI?'Lÿ??q\ù҂?˜ô&Á?ƒàñÎÁ?ï.°í)
!?R§÷³­?0ÂdœÇ?4ÌûîŽR?™æÚ9Kè´?8Fà™é3FGL J0216.4+0507@cÓH˒:ÀIà{ÃŽÀ:v¦%™½À;à€³Æ ?ÃT_Èèf±@5–٠ų@ë"ßöu=¿ãêRn·Ä¿Òë"Ì
¹¿ìƒh¯¹8¿Ø¼anô™UNASNone?Ænl?Šb€èÊä?yvXåfiÆ?ƒË 'ºê³?uBÃãc‰Ð?}Ѧð´r?ï ,¶á­?‡áï𜏭?Wø\ýü³,?h§Ûx¦Á?"õÆÛGþ=?"*C/û£©?î%äÞ)¸?–nsa»g?™u̲úo?‹ÊÓeyf5? æÌŒ§D?V´zº;?îûäéÙî?':4i_wL?sÀ•Ø¦L¾?x}nú¡¡ù?›"=N˜¬y?àX\‰3FGL J0221.1+6059@`³"¦óõ0¿bÿfÁÄʺÀ8Ç`‹[uÀ:Ž¬ÇsÇx?ìy­
U@ºOÌñà­@ts@i|›¿è«¶݅,¿è$ŽßE94¿ë} ÝΰZ¿ïþ¾¢ù¥ÚUNASNone?ÁC³5w?»ÛúP?Çy{¼‰¤?ÃN‹/f^Þ?åÐÚÉ
9?É+!
òT?}‹y€ß.?"yºé‡nS?Ô
u0É7L?ÉZÛL†	É?å¿®utbœ?ÉNJæóœ®?Ê%™¾Û½?°¤ne"É?ÐýaÚ·?±ûçéÕÌÊ?ásßnmƒ?µ³Î¢˜Ÿ?¿="ú¡Î?¬ž"~üÛÙ?Õ‹»d¿?º©ÏSDZš?á'2˂ùf?½5®+ùo3FGL J0221.2+2518@bjª¸¥Î[À@£
ⴖÀ:LÓP0šÀ;à { ŠO¿Ç±Ä'?N¹@
³9Ó¶K?þø…à19¿îÉôYo?à¹*,q£¿×SŠ^ƽr¿äÁ¿z÷UNASNone?ï̸7D?€ÀñøL?<ê½»M–u?Bò	[ç{g?wÕ8—)&¢?€E§ 
¹?îÍox–gT?¡½ÿ ?:"ŸÇÔ?ŽfÀJ¼?´ÿOÁ?›Mè¸Èˆå?îØÙ´æº?Ž;ºp¿^?…A	5ü?tQÌՖ)?šDHzH¤£?‰íÓMòû?îzóO?žbùE%?‹ÏÄMßÚD?‡hÓr5?¡\Ð^"?š"	Á"3FGL J0221.8+6138c@`®›¥ãSø?ä8찗âàÀ8íŒ- L;À:9GMœk?éñiþ÷A@O‹8Wà<@[Ê@«kÔ?ïþːü¿êÐÛøíDÅ¿åoKKq²9¿êõ1ÌńÉUNASNone0?…Þq•×T?&8Ýîrm?°i/,ï¦Ç?¹)%Áå†r?í›`Uã³É?ºù†Eã?"ÖÎ=?¯X¤®
D÷?¶HI…?º»ePÓ¯?ì–f_æ–?À©/¨—?À°ƒo±‹î?¥÷[áK?Ê(³ÈÆm?¯µ˜"Bu?åIÞ7!kh?²ÒŖ;¬ß?»ÊWÈd?³jžÍIà?³©Ô@Øú?©è׿ίü?ê(51Ó?¹éáHŸX93FGL J0223.6+3927@a¶¼œ#¸À4;>šo'À9Ì@Äì-»À;À¬ôÀ0Ý?ÙlÑYÏT<@õ"m/®C@:㟢J¿ä%,º°´¿çS$͔ɿ䝻Ýï½p¿åñè–	ŸÅUNASNone?í´»¶ñu?²I¬?Sþ?›…&±gؔ?¦		Ö\n?¦ñ±84»½?©—¶Y¯ás?í›ò[£¨?´ú?w¶K?™öH j9{?¢šwáv?©Eºê¨¼?­eõüïŸ?íŸHö¡Ï‡?<¹IãÛ?—*>¬b?†AøD?ªJÛv±\?–;Û/®^?ì¤Ô7î}?¦X3ZºI?—È'žnG?Œ9ØÐé)?¹`ϖ˜ð?¤ÿ¼Ì¯ñm3FGL J0224.1-1846@hŽu:>À/ÀPÇÖ¡aä÷À:t˜XPúÀ;á÷Š¸Û¿Ë›éɁ@
Ä)Ùî@3ìŸûÞ]¿âT³æÌÓ-¿éûAÝ΅g¿Õ+s¢JSq¿ècÃUÍ~UNASNone?ï´øÞª?¡‡	•Òs?D=ÕZ9Iƒ?GJ>W!@?›Çr9Xó'?¡R5"é²?ï[,¡°?"EŽï:€ˆ?h‰$ë´á?pú䒜a/?'ŽuéÀ"N?'¸
†›#?í­†¿@#?š'à[Wºx?'k¤;´Ó?€×ü—?«ñÍ=Ž#y?•Ú{K£?í¯Þñ'*¼? *í'Z^,?`©ªµ¤L?aà¿ÁÎo?±û¿Æüù?Ÿü$[S#÷3FGL J0224.4+1615@c$÷QÕÀD‹·¼]êÀ:M®ƒ5ªÀ;©ãîQÓ¿ðò€Á1@±Ê]0ݘ@=½O¿äý×p·ª¿åË¥Š¾Šj¿ã.z:Èl°¿Û7\.nUNASNone?ïØʜ~æ?urVÌÝÃ?2Å.IŒlZ?2q:†Ä?rn^Ûô4?ul)õ?ï¾RGÇhW?{3Uý²àã?J.·úØÆÑ?Ra½wÈ?}'ð»ì?y1ãò'?îë¸E¶n?ŒàîÚcn·?ƒg´0û?rØDÊÊ?™õvoÎ?‡,¼/°–?ïƒ[Cú´?€IAPÒåç?à"þÖL?N†—°?
O/lTH?€A\<ØË3FGL J0226.7-4747@p´Ú¤ü¤+ÀO«ud0+À:²Jj‡À;éï#8ê,?Ÿ´Ð!ƒý@
j´©ÀX@Yc_uÜP¿êzŸ6J¿é¯
Ñ₹¿æU·A ¿ãqÁt1UNASNone?ïä/«žº?q‹
ï€|›?Dt¤t8?M{Ù¸ù™?f³MÁ{'¼?p²ÄJ€ˆ?îÓA`è‹?±™VÎsWœ?~úܗiMB?"‹Ñù´£s?Ù(®›N?­
ÇWi?íÁ³¬,º?–š}<9±ý?"á'ÐM?*éè¯ð ?©ýÃ]sÐ?'£ÚI"W>?ìŸF9Òs?­Z¤6 ?†¿ä!FÒ?"?e ²—?¸A
Ñ­C?¬ñå:ƒ3FGL J0228.5+8213@_"âëC-@3ÿ—þŽæ¸À:INþjÕÀ;ÖYjÕa?¼s¬h@
Èé>Èg¸@,( Z"t¿è§®K=§<¿äø'÷ŽÂ¿êë™ëñL«¿ä³°Šæ'UNASNone?ï–ïG¤2?ª–kl¥g?{^ù¬:pY?Î"L?y)~¯óv¸?ìRñŒkÕ?ï"vò?¡yyºÝ'?ŠNÔT´%ÿ?wšçI
@?*§ÍTs?™ÒDéOø?î!Tª?—%+@ò~Î?•Åö7¡˜[?†"tuQ‡ž?¤;´²é:?'ŽÅ˜ŠøY?í0êbT1?¥£ãW%Í?¢`\ž‡?šã¬sFœF?ªž=<®m? àé+	É3FGL J0231.0+1302@c¤pâÁ*ØÀEŽ'Ð(¡àÀ9ý«®o´À;hÞë0¿ðXþú~@À…Téz@b³ ~O¼¿çV]Ÿ˜a5¿éZ^÷˜c ¿àÀIcÌ-@¿æqâÌÀUNASNone?ïâÅt1;?u}± â©?&¤pX"î?(2.ø¡?kÐDÚù:"?u!Í$wL?ï¶#~jX?gÙ 5}?NÇÑqdÈA?UqR$´¤?€Š½ÉO‰?|+_w"?î¿6ækDH?xzý¢ö?ƒ>ðfGm"?r¥²8‰?žyªÿsÀE?‹z‹\œU?ï3"Ùl"Å?‰ÙGjë™?#,9`ÓÂ?'ö~«šj?™i«ü¥Ù?‰Êc®fr3FGL J0232.6+0646@dNÚfƒÀH¿‡iì-À9öKµ
8hÀ;µ"Ô7û?ë*¬K{I@@ÒMë@SáÀNå¿çŸ?åŒü¿æf ¾;x¿íkÝxG¿ê{çNz¯UNASNone?ï‹~8Z²¼?Œ¿FKja€?€î×|àÂ?ƒhê>°ÓS?xc5§¬à?W.¬cjf?îé¦åú<?­
ʚ¤?LÛ´éF?"(ĄÉG¦?¨>]š³!ä?¦ìN¡¬2S?í>,¶_«Æ? ÛeâØw?£×¬'Öû?"¿yïŒ?¨F-írlž?•GUŠÜ?è–GC?³Ò½À¸nÚ?¹ÕA=‰¼)?®Ä'.W©?À½NìÎà?®ƒVHý3FGL J0233.0+6237@`Ê8›R~@(ŠbÄñ6À9h>­º¹À:²pSO2¿ç¯`Å"i@…&ÉB~«@XL jÓ¿èl÷òaÔ(¿ç˜Oº}iã¿ì×1ú™¿ØÃîÓTUNASNone?ìù¹ÒÁåÿ?º+ª4"q?Ÿ\ހ²K?¥jQFÒÖ?°ZùÉëcs?¶a‹"§™?å2§ñ?Õ96äwٜ?vŸš?£Þ»çÿ?ԓG|^?Ô¾ÑIÙ%?âû䱜ï?ºB
¹Y?¾
ÿ¼
?¨þÌ捒p?҄¶­Å;¢?¶'w1íÉ/?ëû%™K…ç?±X¢èˆ?Km¦l†Õ?U(œ#ø'?¿ï÷ép÷¼?±MZÊ¡º3FGL J0234.2-0629@f-ˆ¤~ÏêÀMf^ê–À:ëLÔÉÀ;ÚY§;BÌ¿È´• ˆ³@÷;á,«?ý¢~ðuô¿ºô¿§¦€¿æqô%‰Û?Ÿ÷*|'T¿Í†•'˜UNASNone?ïð%"æ?\¾{ìíV?Ç-¬éö?ô©éIÞÒ?^ý"Ž?\X'\ëM"?ïÈ×è%s?}€%3ñH?G'à€¹?Q*hR¾9?x¡Ë,ž6b?{W¹<6h?îðG)7x?†a?<E(Î?"²yuB?r2ZÈbÿi?—¶AÕTBš?²&°zH?ï:ú¥o-š?ŽoCg9óº?f?PR.?2MAœ>áÿ?˜…ECÚü{?ŽeOˆf&3FGL J0235.7+5647@aC¿rq7À	Þ×ü«·©À97BL«ª=À;KïW;P8?žô¸[ö@nȯ†Á@Û©Àƒ=b¿ç}D®-¿å¿SÞµ"±¿çÈÛ$¹=¿ìñډŠUNASNone?îxC'r«Ý?¥Ð¿!¢?ž¤åxK7f?Ÿ_ØSR.P?'Rµ™_Lý?"EŠ0њ)?Ýã°Óu?҉ÙCWù?·d×=?µåçã-?ÜY5ö¬w<?И.ø܃X?ë5€"LæÃ?ªãYÒ(jê?³C>ŽE,?¡Wl›`÷?³¼ÏSH¼?žôzé?êÅ]êIf?¤¯bà,\Ÿ?›¯Âԉ?¾"ÜÌùv?Át›´_×?£"G¬©N3FGL J0239.0+2555@bè¬1&éÀ>ö]9–úƒÀ:"Ë@ÒÎÀ;Êry\ã¿ÛºI˜át
@
[,µ•£–@~¸`¿é)I8òԍ¿è—›‡…¿Öïòª	±ã¿ÖaÀ~#¶UNASNone?ïñêK:¯	?e¡m\ÿæ?RǞø´Á?´çÈ|£Ö?[=²b´?ec–€?ïp#2½Ðñ?›?ÁìÛ?jSùKÈí?'^YÄ:1¨?wR8ф?"ƒx¼n)A?ï"ÝrP?…Žþµ†Yž?}–áþÙn=?n2\¤^Ú?—çËÜ[Zs?'æÑý¢©ñ?îq–Zî?œ$ëđó?BõÇìgN°?P7z¬ú^—?¨šÃ?
ö?œ]:ÀÖ%3FGL J0239.4+1326@cæ_ZÙjjÀDÙ5C®«zÀ:
¹üæpÀ;¡ƒB??±¿îÄ×,n•V@v­Aí
Z?ÿìe¾ö [¿ïMQ'Ì?áÌD' ñŠ¿ácH7¸dF¿ãwrt³þUNASNone?ïè‹6ó?i·{iˆRs?5'PÍ
€ú?7_ž2¾,?dÏß"«¯?h++ýu?ïœæ¬òa?…ý¡k5Jƒ?X¼á¦¼6D?h‹›ÄN–—?…®¸Ž¨ þ?ƒ	¸ëjò?ïá1£Ïs?…ö¦3æ™?''ß'²`?q0¶Û	´?"¢j7­o?Ç}×b:"?ï~rÇǖ?ŠühŸícó?[M©qæd¬?f¼ÂÀ?ŒùğÑN.?‰').xŠ‰3FGL J0240.0-0253@eÓ0üø
ÃÀK>ýuâlÀ:T¢Bµ‡6À;ä™/ŽÃ?è™SèNL@­Ô°p÷@€Ì_iœý?ϧïâj\¯¿çWvÜL¿¿ïÔFxVË5?ìý["KUNASNone?ïúr^šò?Nø7îzÔ¦??à–‡ñÖ?I¶vхH?/­-?9꘩Dsg?ï̅tz?€'cm'´?HFÝ­R^?`0<V¹)A?v´j
ìX?zçÙº×8?îWdÎï7?–\7ø<›?–ê̒ÜV?ŽáËËa?ž)k™<¶?€N#tw?ï¼ÏCÈ?‹JŲí?9"^¦çô=?Z¥Rp¾M¶?€©±?Š$ºµÆî3FGL J0242.1-0534@fS—c^t*ÀKûà¤&À:jùYó']À;ãåÇo•º¿ï²	Û~Ÿ@½§¹íÍ@×è€\†¿¿é`eŠÀ°+¿ä.ðÞ¤æ¿âTÂÝé2g¿ïÿZ=†UNASNone?ïð_Vû´ü?káÇOƱr?C	r´ès?L*M™t ?U¼˜À;'¼?i?×h#³x?ï°=æ4á?'TY¿ñ?S•Qä2?Y›ƒÈ‹m?}ã'öA¤?€¾Y¿2jÚ? ï{4?"%S¤¸Ú?•X	Ì2Py?‡1ؤ?–2ÞHû?‰¦2–Du?ïeXþ"/?ˆÄÏt7Öc?Bt,䜪Ê?L+VÆù?'Á>ԕ7¬?ˆB}£]3FGL J0244.4+4745@a»C¬ÄðÀ%Ø?³t63À9ە+uϐÀ;©V)Ø@ž?óƒ#Á%NÄ@]¦^y(@þ€[¯ÿ¿èN›c?·È¿èÚç¤m¿í'<«WL¿ïþ-€IoUNASNone	?Õ=ykWûq?ËäQIÎÊè?Ü0QfÌW¤?Ñ-Q±'h?Í$j[·YÖ?ÉkAì÷™5?¬,SÏ9J?¹±´]»ÿ¹?årI{')"?ʈ("¡ð?ѕìžcŲ?ÆÕ´…Âtô?âY˜t§
?³#µ`AÕ?ÐzTöED?°J9Ïøm?Ťô@×£M?«DBd«?´GíÈ?Xh?§Ä…›5?ê?<Ú==#?¸é4tîê?¹¾+eÖ¾{?°SːÏLœ3FGL J0248.4+5130@a™
9À<ù…'À94´7ª'À;Oº*2Ùq¿Ð籺¢¨·@ûD¸Ã+@‰gÀ-­?ÆáëRôš¿êEØU'_ü¿¼e"¤7,¿áW£UUNASNone?íKۜN̂?´¨Óln?sð\·ÄV?yšqx'0l?´b[ž¬?´Mݒrp?ë\ÀW?ÄA›M¸çO?—3Fi¶'?¡‡ÎÏ?á?¿RÈt:ÚP?Á•UÃDñº?ìKRvÛÓ?¥>4zAß?žø›žo"[?ŒÙA
¹xÜ?·ç~"­XÐ?¢–Ö¾:±U?è5fo}Jo?·æ"ý]?nï[œQA?uel ·^?ή¨Óš•?·ë5ßuú3FGL J0251.1-1829@i;ºKâÀN•6½+oÀ:¥?CÄÀ;Ã}ºŠ?ìG>^ú%9@
b›«—ž?ùëÿ0ø?ïÿ9Ã^ÿ¿ïÿô	N*?ïÿÀ¤Vt¿à¡âDrªUNASNone?ïÄÃO7fB?×Œ÷0Ô?%·Ç®1?0¼¡Îd?|ðš,/mÃ?Âaõ}ª?ï—Ӑo"?œbÑÁ낥?_<:Š½?s›£íG-?†*PԒà?™UWKÒQ?íJìÞý? ~Ò¢ê0?›Æl ŠÕJ?4.åoN?­{ð쥃?˜Úî",wÏ?ìõô(ŸsX?½üJ§7ÊÖ?KáÍ)îÓV?rvqÌÚ¸?¸› °‡"?½ôGÈuÃ^3FGL J0254.2+5903@aDèh3Æ¿Â6év&À9Rk–QÀ:Õf££×?w0Éraˆ¼@­ºÛ³šw@D¾@Bo¿ä¨ÞI昿ë+`Š.m¿íµûxT?ÔÕĀ€¡"UNASNone?Ú;Öñ­8?ÐmpÎ†
?§®Ö¾à?¬còÊ{¸?ág'%ùpö?Ñ҇î…(?µr©S-?ÄýÈXu ç?®bœ³_C°?¼œâ»ÎI€?ëk•Q"á`?ɯ¶¥Žõ?ÞLª¿?%?»\E L›?½üð®œ=?¨Æ£Ý?ÚoV•3ê?º;ŽÔÇ?êù€,>
?¾^³òW?e"þŒ†Z?zØzIT§õ?ÃëV•½²?¾®QˆjP3FGL J0258.2+3555@b¼§›ºÜ
À47ÙUqKÀ:({_ïJÀ;¯è?ïÚÀÓ$‡É¸p@
†ú·Šñ@àÄ *í¿¿éÃG†Yÿ¿ä {Ó·'¿ïûbd¬°€?ïÁ˛R	UNASNone?ïÁóï0£ú?Ž²$'5 ?hG!´ÐP?6®çhÙö?râwEÛF?"_:/
?ïÍ©ïÔ}?z•9Ò¬û?NöØøÞÌ?WUŠåÖóý?uL ‡¥Ã?w½«£À'?íŒöB9•Ê?š¨Ø\eé?—ÝLÄe?…Làña©Ñ?«O
ÀA.?–ZÀÄÂ?ïýÃ/Ó?C3qàñï}>DòT¥^4Ç>rù‹€Pj¶?3—8Ø?C3qòw73FGL J0258.9+0552@eW¡"úÖËÀFk	cV®À9¶3ßWÀ;†!È`?ákÒ]Ä_@
KYN$ü@ÿ9À@!ƒ¿à˜[êȜx¿Ýìß@0¶p¿á+µ¹=s¿æÛì4£"UNASNone?êp䐷Å#?¾»[ٍ‰"?‰)áÎùÏ?''Ų-?Ä©Û¿ûÙ?¾£'áû½?톼îð¡
?«NÏõRº?'ó+`ª†*?'¬P	œÄI?®š›` ¬F?¦êº,ü?쟘¡IÝ?¢ÛÒÚ5Vö?¢	³²é?µÊ͒xB?±þeºœ<"?›±Ö	½å?çàªgïœ?¨LÖh—?§ù$ƒôÕ?˜ÓÄɺã&?ÊZoD[?§d…œK«Œ3FGL J0307.3+4916@bAcÀB@TƒæÀ8ö"#—µÀ;KÒ®Že?Ù¶ˆ™'j
@ÕwQÆX@ÄÀ¿¿ãתˆ+µ¿Ú"ì¨y?¿åʖ;T¿ØË´¨'"nUNASNone?îo\£W?¤=A©¹ç{?‹È†Ç~Ú?ŒÄÂd½¡?¢*Ù??¡l,KÅÇn?êÃä‡ 
ò?Ä -Töž)?—]–ã? z@?Â˯å?Áú¸Àé¯W?ëû}r5@›?¥n¼Åß—?«¢;šbÿ?—Þmè%¤w?²¡CPˆÉ®?œ?å(3Ÿ
?ìZa!mՏ?¦n°b—O5?‹³Ow˜ñ?Œ0¾#±þ?¹¶ž5d?¥›Lîà‹3FGL J0308.4-2852@lÀ6âëÀMèÀh ÓÀ:Š7"D[À;õ½
·éç?Ѹg¡5+@
¹õ¯š@Kª@ýÁ¿çCr-nù¿æ&ÓØš¿ÚÀÇ2p¸¿ïÿNµxOûUNASNone?ïÆíïBx?—܋˜?SVhªhð?qïمFQ­?wýón4*?"! !äñ?ä4
çÙ¬?ËßëFú‰è?ÇN'}Àm…?Ã
¢×#6?ÆtžJ +Ï?ÀíÊ®dµñ?íɇ"Mr?|ÊØÈď?£åær7‰?'(ŒZÔ?«^M§hñZ?"ëì."ÁV?äýø5R?»ª]ւ
?¾B!îÙN?¶¡2ÞKè?Ìçà(Jî?¶v»Jʀ3FGL J0312.7-2222@j‹†DR?hÀL×Y‰ßsÀ:h©ÒÌÁÀ;µÙÅٔ?겸›VL@ ¯Õñ
Ê?ùÿ¤ÐÚ?îR'äɘ»¿Û¯ÈqÀ®ÿ?ÖáëxşÿÖÃò™Ì*¢UNASNone?ïçò\bì?f	üA ?Aúo¹£Ü…?Açↅ?c4™?d™ŸÎþ¼"?ï¤ëD^\?ˆá6ú®Ë?Yx=¦5?bfɗyíj?ƒÊ=d"|?†/˜æáÌs?î<ù|n"ˆ?—ëŸÊs<?–)õ+†ÅZ?‰t
6÷ã=?¡m£SdÍ?ˆiø x?í=îNO?±[ç@¾ü?d\ԇ%D£?|JîV¢0?µtééT]Z?±@kÂî`Í3FGL J0312.7+2011@dP¿Ž`€À?›Gb• ŽÀ:$o±hÃ8À;—¨=¡K?¿ÛÃ5#Î;b@XšJïg?û_¿^Õ¿ïI;Ø?áßN¼sÒ¿ÌЊqˆƒr¿ÓÔÃáÁ¦~UNASNone?ïõŸ½n<"?Yd3ue@?8!Y4²?LíÖÈV?S-
ó?X!AýP	Å?ï¸û:¾?~::OÒ?RÍö˜-Ðì?\ gŸ±2~?~ÎõY×,^?zé¥:l¡?ï3pô¢§u?†*ó…(¤ó?|hñöŒÛ¦?jsìå3^Ý?'w¤îÚc?ƒ1+J>ç'?ï¨mҌJ†?ƒÁh¦d{?6Åʹ;?;=ˆ–Õ;ƒ?…3Å0ï¡?'è÷?íñN3FGL J0322.5-3721@n¾"åÞÀLY@_k bÀ9õM–ÃüÀ;ÞGòù?å>k¤Ø€Ï@.:âT@™* :8?Øj*ÊȪm¿âÓ¶Gnj>¿åß5C}n¿é'l8YÛ
UNASNone?í´­"5¾K?­²¥Ò°Ùî?¢ÄÔ³»}?¢ÛËÞÉ
?¡ðS	†_Ù?£|XtìßÇ?í¼Úª›Ò}?¬2Šà÷vÈ?"Dškã?"߯*?ªM4¢<?¦SSeŽ¥?ì…Xπê?¤4j,hÂ?­ŠpÚ‰?œì™¾MÎ?ª$zq-äÏ?"Ülk¦®?èÓǧ©
?´Éqß(»§?´syh?¢"×Vƒï?ÂwUát§Ó?±¢LïbA3FGL J0323.7-6038@qB¼£n/ÀGç4.ÛµžÀ:|#²Œ¯¦À;àÖìá?K¿ûð ;´·@j‰9Ðf@"È߂\¿åy3Ѥß¿ì¬\`ÂÒ<¿ DÏI'¿ïÿ·`²zðUNASNone?ïÊv±ÐJ?—tNDùÕÞ?;ѹˆsC?I% .Ntó?ytT?—BÐg?ï¸yJ²'?€.õe)?MõHw—ê?UÈ,Yª¤?€[êâ?}›¸UÆ_o?íé 1_@8?—l¾ü??›{¥v³ïñ?Œé(b?£¨*.²}?'²ÇÌä>ë?á«E/?ˆMÓ×;–>ÿ¹æìKm?åSК>?ˆŒj¡¸ª€?ˆI4œ""î3FGL J0324.5-1315@hï?»×²ÀIÖf¡ÉÀ:R\±±¾TÀ;Ó&
UÄXÀ	rö퇭^@
†Nž)Ì@,è…Ç*¿âÁEiãì¿î¿æ¬¿3?kîb†£k׿ïÿ¹±3ŒUNASNone?ï?'¹ £-?¤.,—Çו?K°aKÓ?WøݳaB_?—4ÓXã?£Õ
½4_?ᄊ|šøø?>'¥†"?JårHOÃÛ?VC³µ|?}Hiy‹i?jD.òI?ìÀÙ.ærf? YGXSër?¤¡e™ï?'gÿ˜T?¯êÌ3?°?˜4×5í‰o?ïšë)zÅÛ?')Z{€~3>ã¾c‰Â?ƞ7t}?‰@m±µÇã?'(–y€ä|3FGL J0327.4+5828c@aÄí(Œç?øÝÈgã>(À9vG…À;ûXÑRn?ï0=÷(ã@Âg
€F6@•À8–¿ÙÑiüÀQâ¿å®üd¿ó ¿ì="ßEu¿æÿBpÆoUNASNone!?ÛzøŽ6Ö?Éÿd5÷?Ð'ð,‡?Åy¤w½"í?ÔgEB
?Êó·s(–c?ϧ`÷.ÊV?Í[uf&¶¢?Á`â~&¦?ÀŒºoÄQ?ã¾ɔÃÂ?ÎoCEéã?åÊëØk?´èØ-£«N?½íèõ{?¥ÆfïÁ?ÌÍßÕàӉ?°ýt«"|¤?ÚAAºeº?¶"|G'…?ͦ¡µöÍÌ?½ÝžÆ¯O}?ÖënJ3_?·ËòtsY3FGL J0330.6+0437@fp¯%;ÀD]9–úƒÀ9º~¸lÃxÀ;'ØåßÃJ?ìJ	
šÈ@|Õ@8Õ@ä`RP/¿Ï¹2À`qŸ¿äÖƄDƒú¿Û[kP…ÿ^¿ïÿðH°{'UNASNone?íã~pØ7?³ŒÍS€Z?¢U"ïj?©Ìm4zÊÀ?žå¬ÛE?§±¡^àêw?ë_&•5`+?·( ¸91J?§&Œeß%
?¦TãHÞÜû?¹s…#el?±¼°'i'?è¦ýSË°?±/ä)Ëâ?·à@?¬—¦ìü½?µ_·•[do?¢o¥ªl²7?èT8~fºD?²î[ŸJ™›?°B<'ŠµN?¥‡›{#ç?ƍÿ½¼O?¯óÃ8^J3FGL J0332.4+4644@b¯a¦
EcÀª	EùßUÀ9®?uŒÀ;k|Ìy1?í[µ‹Ás@
c?aì@À}àU•´¿á±²-þÛ¿êŒtª7e¿æËirµT5¿æ»Kô
˜UNASNone?á¼]IøÅ?ÊPéKÌßÇ?°ó'7®¹?°Bx6Ud?ØJ{žFÉ?Ê!ÄSfÝ?ݟKùhÀ?ÐZJ'bU?Á¯ôžbÎ?»ñFŒ	0?و¹·eØb?Ê…=*ò¼?èÑÀQVÝ^?®o	áI¬y?´ÛTq*?žè'ò¿P5?ÂK?l	p?¦6'šðÛ?áø'i#Ï?µˆx`Yã^?Ãð4";8?µ8i[ ?҃娦Æ?²…Z\23FGL J0333.6+0233@fÆÝ/Ÿ¾ÀDwŽ`€sÀ:;à5_]^À;»*‰@†¿ðÏpˆ©1g@
+Ž
{"@'vŸït¿ÜÏ?ѯ¾'¿æ~øù?¿ÇÝ0r9¿èæßé<͙UNASNone?ïÀGí›\"?ƒì·ÈËP‹?4@ò%YÀß?5­÷)yò?~—úü®?ƒ·.ºÒ¹š?ï—ü×Ë ?†Š²+=1ç?XÿN¥m"é?bÝlVÇë?†àà8ŠL£?ƒõ¸­¼ä2?î'€–[y?–	 ä+›?'dëçԙô?ƒdÏA-ýú?¤Qb¯ûy?÷Ÿ¾Èh ?îȖ:dô¨?—áŽ,O?0±ŠÍm?8@a15ëÑ?£Vjö›ª?—ÖK2…d¸3FGL J0340.4-2423@kQÃóà7ÀJÆ)ñkÀ:œ+Àx*´À;ð|_Ìï1?À¤7F,#@
'Ù@µ/ßì5¿årekÐĺ¿Ú0—–£ß²¿äÀ9EñÑ¿¿áð™#ì³UNASNone?ï°éS€KÂ?–h2~J·
?Q8ÿõ'Zï?`[»¤Û''?ž‹!:Ä3?•iŒ7﷟?î™Ú×îź?«r­'âiã?'ƒ§'}?'9\±Ÿî´?¡¾ñ—Iݼ?¤œfg`cå?îmŒ—N~é?'MùuT™?Sî"N?~g§\M?¡¡D?Œ^>Èü~Þ?웟KSN?¤	Ó"G¨?"˜ˆ©	D?Žu"hé?¶gTã{#A?¢s€+ەn3FGL J0342.3+3148c@d
â'@·€À2a"D¿À92»K›	À;,äd™?íϣԅþ²@ôÑø/Ò@5F@V1e?ïã–>§×¿çA½¦ˆÉ¿ç*éy<;¿åGÅ	›‰UNASNone0?ìÊØ°ŸÂ‰?¸üÅâ_®?®Ì™Ï"0}?³Uøýýø?¤…Û&o¦þ?«.#ÐB4\?ìoŒ
O=?¾+}Kœ<î?¨-mtã?°ºƒ1ñ?°mÞ˪?³v±Ô7¥?æédõÏ?²©{'íìÑ?½a¦›¥Lò?§)æïHä@?Å©˜ÝêâJ?«øÙg?ÕF­EwZ?ºª÷º¡Y?ÄZÖŽ#»?¸ñs@!¯Î?àEóÖàèä?ÀLÐÂ4
3FGL J0342.8+1321@eƇçÀnÀ?÷\9¼º0À:z¦ª#T™À;¥ôæò?ä0ÈCiûá@
LØÑÞ?þ‹¾_K¿ò?¯&ˆÀXu7¿Ë
ùЈ¿á®ä^ä¼Ù¿ÞO•vk¹"UNASNone?ï™uFx1?…ã+JÍa?WØtBú÷"?[û?Á=¿?†§ŸÙ™Ç?…
?^m˜?ïC¸ûw0ô?–ø•"¢ù?pÞ¹CæzP?vÌÿ›Œ3?"Q2@ C?"|x¾jA]?îQPdþp?'þ_ã6f'?"ÉÂm?'ùˈ©? †l>~·Í?ˆ);;šŸ‡?ì–ìåE¬¦?£è
6¿?"ÓAì½Ë3?'ÄT«É†?¶ÈZ£(	?¡6ØøŸ3FGL J0348.1+4431@c!Ù©T"ÀD=F²lÀ:;ÔÂeÀ;n=)HÏ?ºŽ›t÷4@-}ns%@5G zô¾¿×¥Á'~iµ¿çÑÚ?üð+¿èduØÊ1¿ÔDRû$¤UNASNone?ì[ÊuÔ*J?¹ER°¥'?£4cÝŽà?¬ÏÅlÖä£?³‡zoæF?³dúÁe¼?ëÀ8Žq/?ÅPœ{S?›KW'æ?§±0†`$¥?À#"8Õþ"?Á&¸PÀ.º?ìF\Iî?¢;º4·?¦"§€…c?–^´øIò?²†_C!`?™oPÇR?é6=edïþ?´FےU3?'0B¦ü?•3sqȍ?Èädb(ë+?³ò¡|"9Ù3FGL J0348.4+6039@aßî$5in@‰Ð~25À:2‰'
ÙÝÀ;± žÛù¿ÓLI¦@
^'í'úÇ?þ4A%9J?ïþ"¯OÖ¿ëÞðQJö¿×<•ì»Ö¿…8…âÀo•UNASNone?ï[p§¾­? t¨a'&Ø?3º €b?9®™h&?"E̪I? ]Žƒ3?ë$ÕÌàJ?Ê[ø%­üå?}é|¢à†±?‰÷T¿¤@é?Â}¥Ãµz¥?É¡OC=ú?íD1…ëQ?¡ê¾²HñZ?Ž	'låÂ?|â:¹jÈ?²AƒÖð? Ñҕë=E?´ï[ô?›³°Ü﹩?+M ·Ú
??ÄÐ0èï—?¤*GRf¼?›¤ú}Dz=3FGL J0351.0-2816@l,@N¤©ÀI:žË1ÂÀ:½4Ùü`8À<ßÇ{T4¿æÛL@
1S1€U¦@WL_ª	©?ëB³ÔáÌ¿ÜÎÊÕô
K¿ç-@µ‰˜¿Íp³G%ëUNASNone?ïÃâ@GWå?€¢ ¼…ª®?`Fv²²,?h`V³koX?u뤃D´R?|µB[ºB?ï»þ-¿ô ?€òÙ+Ó?M¯B~^¡?b@ÚaÕÜ?~KÐC$~?|Ògk(u?î~êi<?•q4·Ñ2?™z†66")?‹>ÿðÃ@º?¡JÎ>Pô?ŠYO¦v?ï]ƒÃ1ƒ?î"+'Õ?A†ÆëÕh?JŽî×Æýý?"Ò9P;&"?Ã@ƒ~hV3FGL J0351.4-3248@m"ßÎ1QÀIs,B»fÀ:eZJÏ1+À;õ¯OäCâ¿Úp6Úîµ@JÌõfžð@`g "I׿è%¯ó´Sj¿ç=‡ëlm¿æc¨]¤n¿ïÿê†úŽ/UNASNone?ïŒ5•Kƒ?¦Uìe×ü?U—V÷/Üé?k\0­:<
?Š?¯ÞG#y?¥ÆÏ ïo?ìR(šÓèF?¹ÇSÈR.?¡ðç·´º?¤ŽK«DÏ?´àBµ"ãu?²8~äV³(?ìjé=?¤N…'0?¦ÁÛàÕj‹?'RÊEBî½?³«ºÇÈÓ?¢,Á–›<"?êHŽðAªµ?³òp>›Ð?¨ùxhø ?£RŠTYõ?ÀŸf$»M)?¯s­ÄA¥73FGL J0359.7+7649@` Âø7´¢@1ÐWÙÛ©À:¥ID°FÀ;þb°Ï@E¿ÜôP‰Û5›@ñvæ;^@Sù`(´ª¿í,#³Iª)?¨,ôÝ¿ä8B¿è‰¸Ÿˆ	éUNASNone?ïÏȕjw|?£C;[?½?q­™x5gV?£D²F?Y¸oJ;j´?[ò*Èo—?ï•s¡j¶?‹ö¤{¬\å?r­"Ws?ví"Bƒw?L¹M¤¦¦?…õSÚ0Y2?îÖ>™Ûׄ?""«ï¹ì?'²jßQ?‹p˶ù¿O?'…Áåt¾˜?…0«a½¥W?ï¦Q¥_X?|ãΓ.?lE¹¢·ç?i4kGš£?~ÎÈÐ~øI?w=؟œo3FGL J0401.0-5359@p'4'¾‹ÁÀG'.œË}AÀ:ÚºÊkÉ}À<:L,(}?âׁα¾@Ý"bô@ɑmä	¿ã8Ûn®¼õ¿è¤ÐÌX*0¿æŒVöq€?ÒPJ¹?YæUNASNone?ïXØ"9?¡†IÞ2j?dJR°Ž¦¦?ŒcDN8úN?Š—fÓÈ? Þ´lh?ïk©c™^?¢)¦'ÚÍ?iEÖt³
Ý?ˆvà?ªŒù?ŽÄ1|'$×?›\#mî??í‹a×±cg?™?÷ÒìËR?™'êeÁÍO?ˆaî4#?ªˆmRâÝ?"0{Rä6þ?îô¤
?Ÿ@øïø?h( ',s?†	~"\?žx§lØܺ?œ‹Ích,3FGL J0402.7+2616@døP›ùÆ*À3"{՝VÀ9Ó÷Ò4ÛÀ;'‰¬¼Œ
?—½Iëêý@\ut cM@.Ðg¤T¿èU‹ûÝm¿él"©¼¿å'Ó¾¬¿ïþ[híxUNASNone?ïªc¯q?†Añ…«»é?jÿæ7"Í?y	˜ÚFϗ?}N5d4ÇZ?~l‹àÛ?ízŸj·€Ê?²ÜÄ^?›þžtz"h?ž2¸a??ªVºJâ6?¬¯62Ñ´±?í¨,æ6ߤ?š.C›ì"Â?¡Œ?)ý5f?‡L‰[ü[?£ðòr"ÐV?r^ªR?êŠàÑõ?ª]*[Ín1?¡nw¨ ™?"¥"ПZO?Á{ö'°'?§É`/CÙ3FGL J0412.0+0229@g³ÞÊl À@¬e"¯OÀ:
㎰1ŒÀ;'Á.32¿'-Q^·ÿ@V±Ÿõ©@0oß`ù¿ç	mý^¿àŸÁ¿ìšr
±¿Ë×2®uk3UNASNone?ïÅϔ€üR?™P<ë]Ùh?o¤¸"'›?{>ë/âÖ?j‹³\q¦$?—'0?ï¹0ꓭÃ?~	¢Ø¨µ?PŸ[ü«ß?WÒ5¯DŽ??³¶þ'{?zù£ìùb¿?îÇäèÒÖ3?Žé'ÀCœ?p‡â[îZ?ƒµ[(CÜ{?–'ÛIKE?"¥xI={g?ï7£JšˆÃ?ÐÙ3§¯Ÿ?L—ÎØÞÇ´?WBgËj# ?˜&Ø5çñq?~#µÿG‹3FGL J0414.9-0840@i;0©7 ÀCMs\.ËÀ:4õIØqÀ;Ï$Ù¸¿æ{ÄА7@ÚAP'Ny@:³ɹȿåªñ)gFO¿å¼;÷k˚¿áû&'ÕŸ¿ïÿ½¶¥UNASNone?ïʦ֮c1?' LŒÀ×?AÓj}F‡?EKLöTÎ?xŒZ;~¾d?'~ˍֽ?ïcºet÷?¹4OãX?g¤…iæ¿Í?qÈ$·p©d?"‰.?Œ˜œnI?îтþüD?–g¸Ÿ?žëCœÏç?‹¡Ü܃Ð? ®r.AÓÑ?‹öTHœx"?îÃt"ü©c?"DNFžo?bGœ>÷"˜?e–£4…Î?¢¤DE÷™?"¯3¿N'3FGL J0415.7-4351@o#zcslßÀFý<£}šÀ9þ¥é34áÀ;ø½$¹í?Ûytß꥕@
T—'hÐ@݉ÿ󕹿àe¸Û[ä¿çŒÁ!¦v¿í.	öV'¿³9¼k—UNASNone?ìÀi*Z¡?¹÷©sA˜â?QöüÚ:?ªl—ŽóZ?²¶¢/k½?µcïy×r?îÐ)p¯r5?²t?}>GW?}¼we'º?˜¢¤ŸY3ú?žbÌ8U?«´¶i?ì}ç%÷WÝ?¢\Yv²Ý{?£(¶"
?"væ¶Ç?²Ž2Áé÷?œ3<.+J?í£Z¨Í¶?­%P;®Þ?Š(VpuÝ?–*÷·üº?¯@?×*÷?ª§¡¶ß™3FGL J0418.2+3412@dzxl"hÀ'ǟfb5À9ÿ9¶ÚóÀ;…vfŽªR?Æîê['Ê@
íyøêb	@úg–
H¿â:|l{íü¿ëÞ0Ss´G¿§¦¹—Úµj¿ïÿù½p¹QUNASNone?çÁ³â;=?Йxѝ14?"yvÆ@ª?§Ø«}'Á»?ΉH:CË?ЋWø‡©?é©|¢¤‡F?Å<ö<ÙÐ?§Ç
@/é?ª`_&vª]?ÃhKrÖé?Áÿ"¹D?ê̅ëàã?«~ëSÝ™?±Üt"ûTœ?šéE×X¬†?½½';¥¤D?¦Î¨'̨?ë	zÉ!¶?´eš:ŒØ=?"q)y¼fF?-u¥~â%?"CßÎÃ?³Îî'÷[83FGL J0419.1+6636@a±+Iº@'#póˆ"À8åbøÜ°À;e¤ëàŽ?ê§cۋpP@(ÛèH©<@~@Jª¿âÎð´f,¿áލf_A¿ã°ŠÕd)¿íþƒŽ¯UNASNone?Ì.Œ;Æs?Áè®
—?æà]8ÓJ§?Ä	Zg¢ã÷?°ŸýÃXã?°~¨K?ȸz‡j,j?įèÀcå?ã-ɬýÿô?Ç¢]׍Â?ʐ^ĝÓÅ?Ãã¢Êg"?àþò³ôWs?·8ê0på9?Ôl%B	W?´Ö¬³wÑØ?Ã+ꬋ‰?¤çHìÉ8S?ÕÞ9\?0Ñ?¹URÎ÷?Ý ÞÅ4ôž?¿Ï®#7?ÊϽµ#?²ÎAûÞïˆ3FGL J0420.4+1448@f|Rç-¡#À87:G#«À9µy1DEªÀ;TÍè«P?êûˆnp@µÇ'`@î¿ÙtP¿âÄMA§?J¿îŸ<=?¿ï"¶|d´?äaU¬žÔUNASNone?îëRFHvÍ?¢ÓßÐ~`?‰?F4@i?"'zg¼•?•ö-W?"–:èóQ?ï*#ŽVç?°w³2æ?|cüjì±ÿ?˜§h"KðX?"¢ "yö¨?¦À†['P?ëÉÎÌ#¾?¥ùW×h?¥{]¡jøõ?";ñ/8Ïï?¶óÚÎ1µ"?¡íŸØ$?íÖ !`4?±Šb)h~>?rô"»Ø?‹É1w°ÛM?°.ö³â¢?±Zøº>3FGL J0420.4-6013@pò~|áœÀDäcÇOµÀ:—Ì9ÿÖÀ;åï3ÿáÍÀqãá'Tý@
š%ۆÎç?ý†Jßø"¼¿ìCÉ»A×]¿Ä|øƒßÈþ¿ÞM±Ôx蟿ÔkËCØUNASNone?ï󼆡€É?V	ú‡?$Ÿeãg3˜?$kRô¼è?Uó'‡ß?Tί	P½z?ïÈ8MÅ
?xùë/¸ü*?FL^^?PÛD8òˆÍ?yÊWQºb?v˧¹"Î?òÝ?"=‹_¢Ç
?q‡t´Ã˜?l`fA֊?•D
1gB¤?€š©3ǚm?ïíU·•C÷?cøàAð>Â**Õ>֒–î9ã?b¥½ê5~"?cŠ¨N°3FGL J0420.6-3742@n	E¶ÃvÀF˜#πÜÀ9[x̚xÀ;£Š:?Ón±Ê¤@凖ŒÉÒ@®m@ .3¿å?Æ ¿ã>ÍI¼ä¿ç†ÍmËNa¿âäӏðµUNASNone?ï	äxQ$?¢3GzQÏ?€ ãI:'?ƒ2ç<W¶?–¹`"6ß
?ž‹Lèʍ?ï>"ÿª=·?"‡²áç¶?jÒ¦x™¶?pˆÏø	õ•?"ø…µé5ã?'GÒ<å?]
4?˜¿¤+?•žQÔ¶?†7u½:c?£ºÇ1ESì?'où…a?íWäJË?¡)š
aU'?ƒî&Oˆ2à?øä½Î?´Ç'–ì£N? ­?óa}3FGL J0421.6+1950@eýR½<6À4¿ÉGNÏÀ9œTŽ†@À;]¹û8ðâ?ãø­âb@Ðf{Š
@¥ã€B…Œ¿ÙæÒ1¿æ}ô}s{Ö¿âö@O6°'¿ì–­™*ÞÑUNASNone?é¦y@¾µ?ÀðÅ´ç>ä?¹1V

PŽ?·R›þ–°?¹šßíùÏ?¶º¾˜À1g?ìEI‡
öœ?·à(4éêM?§I)œþÈ?¦Ú €P?²1ùH:?±[§lêº+?è•Aó!Š`?°Í7/dž©?¿øg]I,s?¥j९vT?»]‰	ª€‰?¤ ]%	I?åÓÿ/wó?®´;ñ ?±¯ew;ÑÝ?´ó]'£?ÏØP†'JÇ?­­¹ü¤Nd3FGL J0423.5+5442@bϕBC@åœÝøªÀ9ü*ˆjÀ:'Ýr6~A¿±-ä?GM"@§ÃÓÔÔ@™€D3¿ãº¥¹ëý¿ìî­…M¡¿Ñ8Áïñay¿ê\ôïøîUNASNone?ß_FTÝ?ÑÛÞ¥7?n'šð,®9?rˆÆP®sþ?àZ¨Â
(ã?Ñ)ÌLÑ[¿?çä%ϸÉB?е&5þ*?ŠËxk'!×?•ÜÊU"?α:c¸ß?Ð-jÝ«¤4?ےògèë?¹ôu¤ÿƒê?¶Ž‰}«'·?¡X•ã½ë?ÞÉk8¬K?ºL'™Ï¸Ê?æ½Ò«ô?Ã!¯¤2§?SÎß%tK?W®j*Í?ÒpŒâÍ4?ÃùºÅ"B3FGL J0425.8+5600@b¸"t¼j@d‰Ø[À9ƒ!
–ÁxÀ;
¤$7îÀþü¯ég7@=ïN×Ô@Çç^j¿çü(ˆÆsÓ¿éäÅ©Re¿åa9Uâ	Ë¿ÇýºDMÒUNASNone?íñÿ¤‹à?³"~)°`#?i'¢"/?lC$Á(™­?¯\µån›?³RjAiÊ¿?횀ø?Á¨¸g^?o؊æ™é?ƒ(¸>îQ9?²0kÃv?À}¬³_Ò?ë=é`™'€?¬ÑÚÞ^ò?¢éŤÜZ?•S}ƒý?¼›Ò(ȸT?¨Bi*ÉÀ?ï†W‡N?ˆfKòfIˆ>Ò$Ži¢Í>æ62сÑ?ŽgõY§ßR?ˆe¢=¾#B3FGL J0426.3+3510@dœP	,ÏlÀ#P—ÈAîÀ9¿Îí8}À;.6Dÿä?ë+ܱ`#›@À;#°@èÏßüª`?ÄE¤—­¿èäKGbPh¿äE"‰£ñü¿ïÿô_
ÄUNASNone?âT‰Ìb#á?ÎòӍÃ5J?À"šlb¸?Âz(|‹bq?Ó
12†á?ÍOYã'ág?ͬ¹ÕaÉw?É¿\á,Ž»?×ùŠ¸Zs?ÆU«70Í?Ú©Š–ÀÓ?ÇòÛÍ¡Å?âÓ¤-ÿo×?´3Ì ÂY$?ÈO†-UX
?¬|†"4?Ìaé¬è"?°¦/ùm¥?Îeÿx`°?°Ú9+?ÕÛ{‰?»dõÆâ'?Úò/"º»˜?¸@9ÿ¥S3FGL J0427.9-6704@qr(õ\ÀCE±cºº|À9cGK,GÀ;Óêçj¿ÜùüP¸@
‹ÝT@¨`ÿŸ2
¿ãõ趧
_¿çt>!½ƒÈ¿åXbü"RÇ¿å\{&kUNASNone?éF ¥3®'?ÆÙ=®š{ß?˜Ç•h|ü?žÞúRõ±÷?Ç̊¾!ÁÛ?ÅýŠ±™ç?ì Ö;qo?"H;G?›Ï‰.l¬u?«úçžàÞ?´mR‰Im?»Öfˆ@,?ëRÕK¸:Œ?¨Â88‰«6?¥)ÎeÍ?'}í¥£ú?ºçAÖø´?¤fœŸŸi?ë"IxÌ?³H֞¹ý:?4A.+@³?÷T#2è?¿Zߢ)iu?²<õˆcÀ3FGL J0429.8+3611c@d"ãû½{ À ނ/ðˆ"À9vygÊêÀ;õÊ?ìms†"
<@
¼¹"EŸ@üŸÀdµ¿ÕË룿çå#üg!Ö¿áÎ+uéU¿ïÿÖµdUNASNone8?Ï>Ô¨<Ë?ÅìTTšJ?¿3Œq·n?¾–»húõ?äIÙGÐ& ?ËyÈ(±á?Ìڌ²Í
¬?ÈÜ<ž	^]?Ô¹°3?Ãϓ«EÙ?ÜÙ°ö•rø?ÆÒ=\æB?ߖ€ 'ú{?´Çd÷¢™î?ÍV ƒ'¼?¯SsÝN¦b?Ѿ/O«D'?³a-A­¦?ÒÇ6Û
É?²"ˆî?Í­p=?µ×sÔ`úl?ÞbaÉ:?·¬ÄÃC3FGL J0430.1-3103@lìÞÊl ÀED¤Ò²ÀÀ:°+Xs^œÀ<
Å󔷳?çß™3©a@LzNP?ÿ‰ÀGƒL?ïý-óáÂ0¿äéö[ïó¿Ë:B†M[¿í€.ž*UNASNone?îÖ¡ÅT³u?§Y-˜y´R?>J§tßÜ?–³–4k(^?"í|­ô±z?¡1GÆÿá?ìÎ\S-Ùz?µµÙçU²Á?Ÿ1tÐßy?¤sv-hy÷?±ÀÀ2ŽüR?­œ{M¬ Ö?é™d=>?°ßC~?À4TÊiÆ?¨¢žUÔ{J?¶ê‹IDÖ?¤"!SÂì?ëÄ"9*B<?³JI¥ÀÛ?¡,Î5¡4?¡ZÛû??¹H‡,?¯(5[xýi3FGL J0432.5+0539@g¿—$tSÀ;ZÀh ÓÀ9ŠDZ¢ãÅÀ;Y»JÄIq¿ípƪÚð¸@Pèà©£@ŽÝŸ'禿åëô¿íU
:ç׿×ÞÞY‰€"¿ã"+Ù-ÆUNASNone?ïܺù²?xnVù½‰?.DãÌñ?;ºÒ½…(?p°ÕŒV™?w‹^ãÊ?ï°ÉR™J?'gü‰ƒ?Wdi½Æß?bE`ã­?€á,
áô˜?€BaØl¼ü?íî*Yiõ?›Wæ(b?‰ã
&‡­?zZôû/h?ª¤—ß¾Ã3?˜Z–xL‰ö?î_ƒ9'Öÿ?˜<_p+f?%'æp0œ?*!Bž'y?©ò¥Wìé?˜	žŊ3FGL J0434.3-1411c@jWŒ½D¦ÀB[hœ¡‹ÖÀ9ñƒ 3ÏÀ;œ£©½Ô¿é •ìÄm@ü'ã@Íÿ|wu¿ÛÀ)˜œ2¿çÚý<´ÄÌ¿ï"ÿž'À?áv×fJUNASNone!?ïó¨‹ñ±?[²-owä`?E÷|ùph?O/€¸z-?KfS?¬ Õ?R֕PËZ³?ï|{Ò°?ƒp8¶^ÂQ?HHK"ž9}?Qmì¤p?{®¸O'à¤?'Í7Lѽ?î­üä  °?>Y"_­?Žš¶KwH?ƒV¼‹	0?šóV@Eî?‡G9'Åâ7?ïфç/­q?zñ@>õq(ŽH¡‡?v‰?¸^&?w(?šÿ?zîõµïæ3FGL J0437.7-7330@qá[À6ãÀA˜À½ÊÑJÀ:6`áÂ'WÀ;Ô}Qœ?Ú:¿ö@ý
WFã¿@Êß^Iâ¿ç4ãöERV¿éæ—S™/<¿¦·äüLð¿àÓ´[x	UNASNone?ïù(Ìw\?o®5L!ã'?/øØÈ?2¯ýCe?I,¨$³u ?my78|P?ï˜z[[+?…Ûl3{'P?X[2\ô?]dK2=å?†Öâõ‰?".ª	2V=?ïL,t$Ç?€,çÔ`þ?v¢°ecù?evtÝÙ0¸?ÑþEb1?|'æ[^¯?ïµÑ?"+¼Ô†Å]?@Í´2 7?OÆzƸ
?œV²GÌE¸?"	4ˆ3FGL J0447.1-2540@l3E¡ÊÀƒÀBØò{²þÅÀ9û=5´ÃÀ;ÓFóÚWпâɽé…Q@
>쯖0.@ÅàŽ6¿å<Ó@Àu¸¿æTþ&¶øû¿ç;M—ý& ¿è
&S?±àUNASNone?ítWkäí&?¹Î*ôög?zCDFï"ò?€'"Àhj?²¹\iž?¸'2¾òÓ|?îðu*?¢ßÖæ9Âñ?y÷«Œ¡ø?Š'i¶Ô?›pî7SÃ?œÊ‹yðØ?í=ÏX(L¢?Ÿ͝+v?™¾c.ݡ?†Æ¾ÞÇg=?¯CØæP%?˜ôâE·?í
µ??¢$ªõsx?{Vû¢?x?1
y)Á?±ÊWåX¥Ý?¡zsøÆÓ3FGL J0451.6+7231@aXÓZ…‡"@1‹Ø¾r–öÀ:F–À¡E`À;Օsš+?æ"+de@
فÞç×j@5.?Ù^Ö¿ê7þ¥ü˜0¿å/–¼¿Þ0‹"iAô¿ê'/îÀ_UNASNone?ï>‡QBå?ˆ<MæðVÎ?w"ŽZøÒ?wäÒ|29Ò?zB™É"Ð?żøŽT?í¯hmvȁ?°,Éƞ1?£j5xJ$u?¡z¿l'[Ô?¡ŸC°IS}?¥Gb7Âü³?íg/@é?¢û5Q_ØP?¡r˜@XÆ?Q#рʒ?®³s¾«?0—E齪?ëÐG4Ç{"?®sBÙ,?®–2n?¤aÄ1?²2­"}›n?¤B7Jr	3FGL J0451.7+5722@bã©æî·@ £›ˆ‡"ŸÀ9¸ÀÂÓNÇÀ;n:©I:?ÜRVMƒZW@
¿Ñ2œ_@䜿¾ÇQ¿ïµoŸf&?ÐXÞ_闿ÕÚ`:Ê£Ÿ¿àèaÓ¯•UNASNone?ï€Tèì7?'(ëÁ/I?z—$‡Ö(Y?…0FÒõ,+?'Ÿ3·Ùݾ?†2_¸¹?èoz©€?ÇÓÛlÇëW?±0r$!ñ?³+$o‰‹?Åb
paz?ÃÊïÇËr?ì¥Ú%ø°Ñ?¤	UÚP‡¥?ŸnMhúå1?æ¾@³?²õ›uûÀ+? ÚXû,o^?èç!°±P?¹ñ×4ä?¼IÆ£~D?³¿¶-¨V?¼¶­‹Ö÷=?²¨c9Î݆3FGL J0456.2-6924@q‹öy|ÄÀA¤6~ANÀ9fÁæ¯ÍÀ;ŠCV–åŠ?ôUü¬
‹@!ÓÛߺ:@vQØ7?Í6;9¥¾¿é¢<²I$¿å`î¦L–˜¿áB#hºÔ}UNASNone?ëw!+´ãX?¹'h÷²
?´_	Š±Ö5?³5­óÐݍ?¯ÏÚ/N?¯œô É¼–?íÁïæƒýê?³nœp>ÞÇ?'ÀLðØÕ?¸eóy`?ªÖ¡qG´ï?¬]:Rý?èöGÄÉ·?¯ŠýȍÅo?Â	ƒ»Iç?§¨çäH?»ÍNºcy?£$µ1çÈ?æ'G§.ì?º_Åù*­M?³¾TÝY?°ê¤^Í?ËÛ¹ºô·)?¸¤*ua¥3FGL J0502.6+1759@fö©ûçl‹À,~$5inYÀ9¼R¯Ð<ÄÀ;@½½eP½¿øŠÖ/¢!@˜‰°B}~@TZ 4"[¿àɪÄöOä¿í¢ý††Ÿõ¿æb"9éŽW?ÒZðiÃUNASNone?îûO'ÿ}<?¢
E
.Ž?dDW¶¬y/?k»2*•3¥?ž
"©:É=?¡tP,ðœÏ?ïÄòÕ7‰q?èÜ~[¿'?RnZ}щ?[Âåš
?xêþޛÓy?|*º7J~œ?ìkà.ÿÖN?£BÙ UÃ?žeÞe+Ùð?ŽOܟ
Ls?µ†î¶W? e=FBæ?ï8£1ã¼?…îÀ\¢l>Ù.@…ÜÀø>ò;Ãϓ‡Õ?ˆ®±kvUR?…y07y3FGL J0506.3-0357@i+IºÀ9{úLaØÀ:©­
åÀ;vj!
?ññüÌï²U@
sà!"M¥@W=ÿjþ?ïøñ¥8"¿â4z/"bë¿ã$–-º‰¿îL‹Ç§|UNASNone?Þ¹"™@'ž?Ì®û²ZѦ?ڊˆ]´š?Íô+!?ºïŒ$+Qw?»}À‹#¹[?³Š¤}é±1?»Q/Ûï?è‹ðȕ<%?ś\¼Öê?Ä
Ꞷ6Ó?½-ÈÌ®—§?׸CîœD?¶º›þ"?ÛḴ`?·˜ì;Û?ÉùN‰Èd¶?±
\R­ˆ?³Ï¹ƒ§A·?§Léì×ú?æ/ac,âÙ?à ­ªw°?ÍZ±xÓÂ?¿"†`"¥3FGL J0506.9+0321@h¦$žDúÀ5_â'@·€À:Œý­?hÌÀ;»*VëŸ ¿ùkm´3@Eþw?üމ€Fâ=?ÐaÇnÅ?¸*Ùô,׿ßAׁ[µ¿Ý&ÇojÆóUNASNone?ïÙ\§Dš?qœÇpÜ~`?QÑë»)d?WÓ<½Ð?mºc5Ò5?oeªugõ§?וֹPßFÕ?†çm*ýÅ?\Ó~O-ã?c&
ML1Þ?±Xde!?"'Q×>?^m?«7Gèâ+?òç–Ä…?€áT7«?ž—÷}n@è?†³"Xµ?ïb›%c7'?¥:Š6?< Xïmù'?E®Ä'žm?":ïÛUö?bp‹CÀ?3FGL J0507.5-0906@j)ˆe"¯OÀ;0÷Do›™À:w©"ÉÀ;¹/š!~Ö?2ÏO§°k@S[žnH@ÀÍÆ¿à£ûiº¦¿çˆ¶xU.ä¿åÁȅÑvç¿Ø¹û{ƒPyUNASNone?îO2±#}6?«áŒS;c?ud#HV?~Ž!Å"
?¨`P"½je?ª£{p]f?ïsø.Ew?'~òT>Nå?j.e|œÚ?tp@$(5Ö?Œv[{9?Ž˜gab:?í¥8<­´?›?Û%mÛç?˜ÈX@*àú?‰9¹y~uÈ?©HSl´=?",W'ißì?îQ¾þm»?—Ê	eC[ñ?d	¿ÙsÕ}?fKÐ#W»?©£tX?—q…iÿ Ò3FGL J0512.0-3737@n0mÚÎîÀAˆƒ¡	ÐcÀ:¦í_‹ÎÀ;æ»:Ôe?Ér¤|‰Ð@
u>mÎå@™Kãö	?ïÚÙÔ¶êÒ¿ê+ýw˜œ¿æ
W	.Û¿×L…ϸ9˜UNASNone?ï›Ü¥"zÌ?Œu¿´Ñƒå?P•Wnç?SÏÒÄ['d?‡Cüv_Y?‹ËíQÍò?ïz2?"jø.+.l?c›†ù2?x4eñÖÔ?Œ‹3Tѽ¼?2fP0ØY?íÊ=ŸT[Ž?˜xŸ®DZ?—ùØ"理?‰å›ߌD?§_9ùBsY?'µÅ™Î"Q?íD*G+j¦?­'•¸€7?vp 5±üÝ?|%7MÄêL?´w«ÃI‹?¬ûã@8±3FGL J0516.6+1012@hû¼¾bÀ/v(í_ŒÀ:cŒT6¸úÀ;yÇg2>A¿ÒÚ#ޒ®@Àà"ÍR?ÿþî_ċ¶¿ê…³tG`οâÔ¤::¿Û¬³Ì9˜Â¿À4?¤ÓUNASNone?ïñN8'Z?`pmüåêé?0Ç>>/°X?2ëþG@Èb?Y2*%aË?^Ò8óÚ<?ï¬nï±ñ?ˆ7–F¾?[ó} ?e"årN…·?taU?"õ2g«©€?îéËö)l?‡yNÌwÁ£?"+[¦pË?rjÔ"'?˜°Ó«Fò?ƒWLeL©?îãWK'?"òÏùç¯?2˜@Ó°?>óÌ"aí?¡¦€1?"èÀ¿E0r3FGL J0517.1+2628c@fSµIùHVÀvvþdŽÀ93PdŒÀ;}#AM¨?އµËYÓ@@ó#x«
@=ô|ô¿âØ(š L3¿çŠK}#cª¿â‡ê©›^/¿ïÿòh´UNASNone%?áOšb"È?ÏN°Ømû?›Œâ¥Q{d?¡IDº}¡´?Û§ýÞº?Ïzh¶¢ž?ÛË<þ?ʓ¥ÉI2ß?ȏ¯ƒ07°?¼§xêÑd?×ìë@PÝ%?Æ#›¬ê•"?â-ê8 ?¹ë K«Ûø?À½o÷4¬?£í»:ç¦#?Óu=ä/ôl?·ø÷âÏÎ?Ü`Ôêu¢?·çž!™?¿¢e‡?®JÁ<Bó?ÛØÃA<(˜?¸+¡e¡	½3FGL J0523.3-2528@l†wFˆzÀ=ӌ†‹ŸÜÀ8£¼:®Q¸À;iÉü7ôc?ðî[Ý÷A•@R$óÅ@;ÿûù5¿â‡¡1h'Ë¿àq•¥ ê¿áUôúâ¿î²"ãøõUNASNone?ƕKyÖ»1?¾Îo}ÞúW?ãْ®š<ì?ÈQS÷™?ÊiËÀQ"?Âø7AÌö?»¿%¶+#Ç?¹Ý$¾ ?äôÜ) '¡?ÈÒÐÉT?ÎLü€hc–?ÂlÅÓbÝH?×}6£r\]?¶Ëëqbh§?ܽU:ào?¶¿ú|û?È䥆j?«ù‹W•?Ñïð½ùñ?¹¯;ÉÝX?ÝßK›@‹+?²IU?Ð0æÆsä?·[&–''´3FGL J0523.7+3328@e´×
=p¤¿÷"'àÙìÀ9;þ®Ç(À;#Ððx?ÁÛøCžu@
E¤—yƒÐ@b †ˆE¿äŒKÑaæ¿éè¸
"'r¿ë3R¼ ¾M¿â"3í~"QUNASNone?ã EYœ??É|"7ôyä?»NbL
…?¶yèi?ÒëܹĨ?ȗV™'?Ãgâ¾Ãæj?ÈâCËÞS?ÄA¾Í×ä?ĕ0(ꔿ?æ!6à›m?͓ˆÖ{¹O?çË{éÉ'?°ø9Eá"?±*1vÙ?š"Áf'«?ÈQû@ 1?­ÀÅ7œ\?ãU§ñÕo^?¸'*á$¹¤?«!›‡?¥Üfô? 1?Õð3Ñ?¸"¿ä/é3FGL J0524.4+2839@f7…ðoiDÀ.çğסÀ9SS@ï´XÀ;5ÛNoϜ¿ñš%ȼqá@ÌwSH§d@þ[`m~¿ä ñðÞ¿à(çY.ß*¿ÝC—ñ	¿àø®Ž.'¡UNASNone?î×è®!²#?Ÿôˆ–fÎ?l­œaŽ!?gzäkŠ$¹? ¶£4Äå?žéÇpìON?î,<
A?±f#'˜ú?w¸S²Ÿ?†w²¬qè?ªE4œ›å?°'Ù¹¹?íªôÅÉ[7?K€èvûÑ?•gù!®P?"¬ùÅ­f?ªÂ¦Ùud?—9"¿Î^?î¹þ©»?'{""žK?,@û0K³µ?0ªô¶5?¤CÔsÄ_?'n,ˆû.¯3FGL J0524.5-6937@q"Ë]ÌcñÀ@jq¼Û¾À:VýŸÓo~À;šFfޏ?Öà•©Ay¿@Âԏ‡?ú"YwI8?ïíNc œê¿Ýwúã`¿à(¨dQ}?Ì@´Ê'M	UNASNone?ïËàlî¼?w}w‰:q?Dð9hx!'?IÃn{{—;?wqïœy?vӁŒÌ$v?ï¶az·u?€7É?Qpûðq±?XQî›âÜ?€9ñ½T?}=£èVµ?î…%(?Ïé­?'mpt=?Þ(âOÃÞ?ñýî
ýì?†	R¿ËÐÚ?îJ™[?¢þHí<•<?W¡CŽÇÈ?l‡÷WD?ª™e±ôo?¢Æ
K¢X3FGL J0525.2-6614@qD¾aÏþ°À@¥ÌBcQßÀ:ëíúCþÀ;¤ß³Y^@ÀÊJHùn@ ]-X@Ý<à†(?ïóšÑýä¿ß(l\ìâc¿ãѾÓS¾]¿Óâ'–¶ªUNASNone?ïøùw.¡Ï?M'û'	Ð?*¶¤#㝴?.ZKq³?Elz<Ý?I(\òžL?ïÇë-(\z?x§Rm"z@?IâG,?s?S"zQÃ?xÎ ‰,;'?vPãg°?îÑgÒb'Õ?‹Œ‹<Ë?k)±ã?~à±_\¹?—|Ÿ6¬{?ƒw´iøa©?ï³X½•Ë?'·,m9>ô·×³›fD?.®ûí?ƒt̀¿¯?'²g'Žù3FGL J0526.4+2247@fÛü;OagÀ¹¹"á£ôÀ9q—Å"/À:Ç)óë?Ýa`r=Ï@'üÆ>@<wà6a¿ë>ñöZ˜[¿ãô‰»fY7¿ééY³$°¿ÈŒÌ¡Ù¯UNASNone?ë½bÒ?»K	µÇ
!? ŽXªˆ$ ?¤^wì™?¹Ð@"*ýi?¸ðÐ"Çv?ì0%"`n¤?Á«JD6&ú?‹€è?þ¼Î?—/ºÔ¶Ï?»¶Tü³C?¿YùpÇÄ?å6"§	´?·ðñ"¶ä?¸í8!>K?¦,­¨}íŽ?ίQS(³j?´ kö0,è?ë_xҏf?µÚˆÇt_?k¢WþuÈ?v\€J¤ƒÉ?Â"UɯF?µ¬Ò	¸/p3FGL J0527.3+6647@b2(õ\@1Ä&5ïÀ:¼ÆŒ@ëƒÀ<Ü<¬X¹?Õð%cß@àà+yU?ý T "žX¿ïy<G׎?è«ûújr¿Ç4A¢D…¿×СõØ<UNASNone?ïóNs?…ø²o¾à¤?C›ïï{ƒ?NÕ&Ôu.?N"ÕÏ@?…×ËC!Ï?ïj3ÈÿG¼?–cù}™…£?{9
câÀ‰?~üƒðÿî{?‡ÖˆŽ<°®?"༖ ?ï7ޏOÁ?…ïx°Ò?"_ –7¢?~€u`…Î?wü‹¢XV?{_×°ÚÇ?ßvÇm?ˆ")zŠu?{©#@'MZ?|cQÀÞ?í
ü~?'ƒ~9ì23FGL J0529.2+3822@eFÕ䣃'@v @hÀ8éæè¹À;+%Â1?ï&gâ.@aÔ=ÚV"@D¡àe¿àH0…PXտ馃('ÄÛ¿êâ3ß´
¿âxC*¥UNASNone?îW''¿ô?§Óq±LÓe?–7<"!|¼?•› æqK?žÖ'à'?¢)´y­¿?Ý.¾_|?ÔÈkÉ*1í?­I8å¶wð?²|ü†2?ß(Þé´ü?ÓÚ'Aß÷?éfÉâƒf?¬Áî¦wµ)?°ÃH18´?š«ó4å1ˆ?Â@×ÝV?¦åø؇(E?åN&Kü¾?·CØ)àî'?´:ŠÎ8':?°ÔÖYÀ/?ÐU´x_Ž?¶Mԝˆç3FGL J0533.2+5944@cõÐúY@,8ðAFmÀ9·´Ï€tÀ;"A® 9?ôw¬NÒöÝ@´¨€èß@¾?–Bø¿Ô:"´`"¿è
‡"¹ ¿ïÿ"[}em¿äüèjÚaUNASNone?ëùYq9Þ{?¼¥?"ÇRÆ?¶oHjeü?¶RÉ=Ø?£ŒJ[L[?©ßtôþŽ0?ë_úª¨‡%?ÃìÉÚñ²?²BÅB0z?¸ïÏdBùž?²éçåy–b?·t®m?è#"Eíü?°™˜Bsu?ÃqòdǬN?©†zŠ‹Ž?¸Ã$A7ˆ?¢ØSë+•?àüìmd?Å£ûnÅýI?Ö	Ü=åXn?ɔ—Z¸h
?Á¬SÓ·™"?¶ôKArÏ3FGL J0533.8-3754@nYcˆe"¯À>âôðØDÐÀ9ñjÉ¢uáÀ;ÇB??°ð¿ø«md¼@4¤m23@¾÷€—:¿Û·çÉ¿é$ {ÿ¿çô•qIw¿Ão¨{×\UNASNone?ï·µ—øƒ?yr–&gƒ?YGæ«»C#?aHF$˜ŸÏ?}Ó:YíÐ?:WX*œ?ïÆX&i?|cª†?K'9ùی?S! ~°?ya®-"¯"?zD°L¢1]?î"6Õ?â-Þ®Ò?
Jnˆˆ?€L¿Dõ÷?ž—6á?ŠHÁq?ïÊåo·ë-?v:^°¶>ìS°~´²>ý¡ü¼Ë÷Å?z8z2*j?v\Ÿ3FGL J0535.3-6559@q=Øâe,À@("_õIÀ9ÖÇÉWÍFÀ; dË[³…?¿ti"Ä@Œ!Ûé@˜¾_쥿åèå}C£¿âíɽJÏ¿é¯DI8¶³¿×?°=†/UNASNone?îk7)(~ø?±J"!Â{?€3Èr7?'F*#[¥"?¥FÀ{q4?®vÂðÔG?ïv6‰"ì?'~Bñ13?e½Üã7‹²?u³ _Ãô?	;$Ðâ?¯7~D~?íÈέßN}?œK»w÷"?˜B|Ì~‡?‡^(ñhXC?§Q×$Øâ?"И5»Ì(?íò-º†º+? 2mXðx?s¦…ò£—þ?xù¿ðG‰?®hS™?êH?ŸÇÝε'3FGL J0535.7-0617c@j=pdìé£À3¯—Ý÷wÀ9Kd'`˜À:ég¬·ƒ?¯+«ãõ½š@
¾‹Õ‹¸0@+Þßsîd¿ãb¡Õt³~¿çi¨$*¿ëE|Ђ¿ÓÕ¾î'Å?UNASNone1?Ôå9žM?ÊÃqué?¸há+…†?¸
9,žÃ?â€c½Ç€?ÍEBê,Á°?îñˆ¯A3?«•µÕPQÖ?'ÐÛzóÿ?–ÆzìºH?˜tÁ,ÙÅ?£ÒE3Ï÷?âÅ\
L9?¸%½.
¹?¸ÛÑ"_&ç?¤BȎ$Ò?Ô>èÿMÑ?·@ëH‹ç?äû
¢-èÓ?¾¾ÛºÊ˜Ð?ˆ¦<Œ%?:àÓf²?ÕD´šÂIø?¾Â6"ºU3FGL J0536.4-3347@mÉ{Ç÷zöÀ=o¼¡ŸÀ8¥»^æ?eÀ;‰al+¢E?ïÔ$
6°|@5"×ëŽÚ@WQ­Dq¿åøó	*(Ñ¿åù?®/—Œ¿âîü"þ"Þ¿Ò¦°UëUNASNone@?ïü©ý9?<$´r®g?°""fæµ?)‹YÔ¹?8î–VüÁ?8è®ìÆuò?ï¿úœÀ?|÷u¤{@"?P·—À¢²V?V5õ ê?{ÔËAwì?zƒѝ;ß?ïU;€w?‰'NÝ?ƒSÐ0§â?xZÌòŽa?"ËÒ7ם;?"
ö^òðï?ïÅÂàm?€¯fJú³'?&_…vÎ9¿?78Ø/ú_¿?|ÅzòÙWã?€Œh§ÆÙ3FGL J0537.0-7113@qŸIšé$òÀ?ŠµÃ›Ë£À:'q^-À;'lSq?ׄð4m@/ÒxÞ8@Ü )€­¿×
ú7œ¬ý¿ë³»õÔ¿êΚr1 ·?¶:,µÎU#UNASNone?ï%Mʃ? Ùȧ¦ªn?r¾w{'ÝQ?zY'†}À?˜¸86?žýÓ¯:³?ïoƒ‰n=?•©ïv?aŒWE\œh?vîþÎÛ?ˆA	LMIy?'Ó}W±WÖ?ìé½±ƒd? @
¢ _{?¢¶e°üp?"ZúóÚC?®­¿É-H?–Óõ¸x?îNV?£æaþÐ[?b9ÁÌH?smSé1‡¤?©ý«Rqٞ?£™?ù£)ˆ3FGL J0537.4+3604c@e ¼¾aÏÿ@h›_lw"À9ƒÓQKL/À:à«ÁºJ?à ¹ü*@
ÈQÉ÷/w@+ œ'­¿å ¹8ùÏB¿ã³Ó'7X¿êŽJÂ,¿Ý—…Ó>+	UNASNone ?ÞÐI?Ô?ÍúϘr±?ÉwÎðM?Æ×zA '?Ôt<™§H?̶»eôÑà?àç*3vD?Ñû´ wèª?·k†©Ã?¾šÎz¡¼â?ØVÊe)	?ÐMd[VÔ?áî-Ç2.s?¸…n¼#Ír?À÷câZN?¯s¿î•¤n?Ó§ò€n"q?¶(ì.Ìì^?Ö¬*O­nU?Á×)p/§"?ºf)¨¦Mž?·ëŔµ²a?á]%£#?Ã2Àº@ño3FGL J0538.8-0341@iû}¿H€À1Ò=p£×
À9™AÞËÓÀ;2qúï?ò2JˆÎ@ž'‰±Å
@ƒßà›¿Ùb\ik<¿ìWG†ôž¿çq6Аj‹¿ïÿp'|¾UNASNone?ãues»ûD?ʏç!ž÷?Äý¾'R)3?ÁR£lõÿ?Í,«ž½éÄ?ǵªêgŸ?ȓ8,±)?ž1Ýcù?ãµ>	ëP?ÈôYý}ˆù?ȘÜÏ«¡š?¿Sƒç•?ࣺ—'ã÷?´)‡Þ¨åJ?Ñ^Q€-?±Jm,ò;Ú?Ê´s `cÉ?«£çqÜrB?¼z²tü?§ðm…²é?á1£Ð>?Á:¥™Èý?ÖÁ¼&‰?½êsB})Ì3FGL J0538.9+1646@g³&¿‡iìÀ£¾"åÞÀ:ütðmÀ;t!퐑³?è«ñàØrr@ƒU@m-?þ@^_0çÿ?—µo	¹lg?Ü'§ÂYßοØeo™H™¿âÄz\¬B-UNASNone?îÏo‰š¼?¨C}í Þ:?j~Üá?p†&±›?¡n6Þfp?§M殆C?ç"Ë}æ¶?ÍD¼%ã¯[?ªôΓ(?­Þzwú¹æ?Êïžc¦ï?Èз;÷X?íçµcð«¼?ž>-v?kB?–=E­fñø?…âa§™sœ?¦fêAË:?˜8H)R‹§?ë"3–º?¬ª0þMîH?±¿L|¬‰D?¢PI•?²†¥Ï?¥ÎÊg:â3FGL J0539.9-7553@qô¢}ŠÀ>–~
ÇÚÀ9ÐľáQ¿À;Â6âëC?²J…^t
±@SIÑ«@š'@‹¶W¿ç¼ŠM²v›¿àÕ6Ó@O¿êÉâ?Xc¿Þ~ØdÒßÙUNASNone?íí¨ø˜‹?®ãêÀë	?˜"Ænkh??¡£H®{ý]?¤ÛI@Ã+?§Q܁ñå|?ïìÁEZ?£†þ¶-?{|n"!ãß?Šýu5H+??™L2ŒDß?݋š!Ð?í_±w×Q?¡2S,ú¬Ó? ­éôˆ?ŒU‰¸! ?«D+š«?š»Åò?í–SÊ%äI?¡éTk?ˆY3FZà3?‡¯õÙŠ?°B;F³? ƒ·Ëh»3FGL J0540.0+1208@h7‡?úÁÓÀ#¬U!š"{À:
ï°ýcnÀ;iþûôÅ¿÷÷äXÍ@œQþ'@ÛQŸÚÑG¿µf#@9¿ì{
jð—¿ÕF"¶U'¿Ó 'ü¨mÙUNASNone?ナ<)ø?¡ú…"??*a#J:ú9?0šâ7@ö~?êXØ,?¡j$ô¬;?ï(¢*gX?£Ÿ
¡_ë?d¬ùH]Ó?sÒøo?˜VŠ	F?¢¿÷…ì=?î~üËØ~=?"u|@²B¾?…Çú‰h>q?wPs¾A?¢ž4 –?'+3á4cT?]Á*Š?œh•¿>ÞªêÕÜ^ü>ï+×–p?ŒŽÓ2Z¡ù?zðÏø,3FGL J0540.8+3503c@eÈ}¿H€@Þì9yžRÀ9QؗÜ*8À:Ց¡}"ª?×týý`,T@
ßÈß'·@* À){N¿¨Q¾N.â¿ë‹Sß¹¿èҘ–dZó¿á+k4›,UNASNone0?ÚÂZ—øD?Ì¡á0=± ?µ@¾	Ïò¾?·~$¤èQ?ßíviô?Í÷*0KÛ?ൣDŽ L?Ó ás[é<?©FÄöŒ?±âîB>¨?ÛqX ˜?Ò¤ÄxH—'?ÝõÞràÈî?º¬ŸÕÿ@s?½Ë
£ƒ3?­•8¸Ù¸??ڗ_vVF?»vLk<ï]?ࢾ™íå®?¼GôuXæ?ì–hUJ?˜²C—‹P)?Ü꽯Q?¼—«¹â]3FGL J0544.7+2239@g(-¡"ú×À"ôß:›À9m"š\7À:Ȫ-e"Ù?Ë%Ì~"{‹@ûäêû¶ð@ýÖàL'¿ëd¯N"¿ìiPjjq¿ÐŒ÷£ÿ½Õ¿æÝÎzªsºUNASNone?æ†m¶f¨×?Î,O3ëó•?¥7¢?^?‡á¸‹Ü¥‡?ÒeúÖ ³^?Î"ê?àÒ4O\^/?Óiˆ¼@T¿?±ÒXL§É?´¶}Ñ4'?ÙçNQ[?рµc'ý'?á~ÔH¶—\?·Ì''ׇ(?·€âRi	7?¥}ßÛ"v?×"ÙøŽù?¶Ã.3åi?á	ÿM"qË?ÆU놷 ?|\¢ÿQ?€¥•±ˆ ê?Ýy¿ò¢m?Æ\0<fdÕ3FGL J0546.4+0031c@iœuy(àÊÀ,Q3ß*À9g<kÁ:À;!1ZL?ëj¾ÿs'@Îìt‡ç@@ŒTçÑá¿ÞxoÖ:ñ¿ç–¢ˆƒ¿ìxªô_ãÀ¿Ý)1þûLUNASNone ?ípHë;`?±µæœ¾?«0ÔEÃ'?«ä.¯Ìb?›•U{·? q DÙû?î~.ފ\D?³½bŽÞ$?‹<'×pm?œ)î1ŕ?¡Mña~ '?¬ËBé™?ëÈ¥®?¤ä\ÕÜã/?ªA‰‹Âó?–úi1váä?´šQýƇ?#O£‰T?æ&–i"ù1?¸y€Çx¡²?«‹Ý£R?«úCH^>Ê?ÐAoñT™3?¶Ûì—ç¬3FGL J0550.3-4521@o}n—OßÀ=H¤TÞÀ:´ƒ)ìÀ;¤B"ÏÞÀd&Æs@üЉż@C )"¿çbò†ßû¿æÆ'Ûjþ¿ê¸NÉøÃ1¿à"}ÊþcUNASNone?ïõqËù?\'rŒBs?@âÜ>u?BŒÐ‰¬J´?IY'bÛ?Y¥'NèX?ïÌýè%?x'œÄyW?Jt8øn\i?Sp©¯0?v¯ùìã!ü?uÄi''&!?î¼KàML?ŒÕÜb˜?‰àEÙ×êµ?x×5bj>?›Žs—
a?†>tfWŽ?ïè"íe}?nÙ6†­¥l>¾tA·Œ>ìÀ3"©¸[?gÞ€²_Ñ?nÔ»¼'úO3FGL J0556.2+3933@e~P]¥@7.jwÀ9-—ïunAÀ;_	ðCÊZ?Hږ!\¡@¶†ü#»@¾| aõ>¿æè'Wގ@¿íbääúƿꄉðŒÎ
¿è=¡íêÃrUNASNone?îãõ&=Õ?£qdK#6­?ˆJK_­¢?‰NMÿ*«?—\5t"? x¯ð±÷O?ê´ã­§Ð7?Â÷–e`ʂ?š½ý­i?Ÿ­ÍVô.T?Áèù¦¡	y?Á'Ȇîìã?냇®Ëð?ª÷ôõ?£àt9wX?"9AëY³?ºWlä×?¦5"ùK?éQ1ùs|ç?´¨ÎÙâÍ?£Þ_ªÎfà?›4íVš´L?Åà/~r¬?³Ò§'p3FGL J0557.7-0720@j®›¥ãSøÀ.}Ñ¢£YÀ:->9 ²þÀ;oX)ŒÁD¿ðä/,=u¬@ü‡ÝÚf=@/;ßÕA¿éâ¼"ä;¿Ó õjÈS¿çà´¡ÃðÁ¿ÆçãUNASNone?ïèÁèϋ¹?fŽÏDðÎ?XD·ˆw?]SìÃ[\?V7_ÙÒž?Y²ᶊ?懲/ðþ®?‰ý½Ç:Û9?^FsäÏÙ?m€®KØÏ?"sõCº~?…nånµN¸?î5
®ÖI°?'Û'§ÔÓ?•;Û¹…'š?"ÌTêÚc¬?¢g5؛¥?‰ÜÃ{""?ï
¹<?"}7;ôs?9¸7¡9Xz?F#>cÜä?žAï9úú—?"pkã´/3FGL J0559.8+3042@f!ê5"`@~½à ¿(À:+0/r´À;pê‹út¦?æjÞu–°@
N½u@ô½?û`zßDH¯¿ïÿö(výÊ?ïþ`  =Ú?cÝåÉQÿ¿Þù…ét´nUNASNone?ï¸QîA
"?"5‹2‡Ž?\™Œ°Û??b‹…Ù?|°Á¼Lþ÷?·z­?ë[æéÆ1¾?ƳòÁ6ü?Ÿ7R&<?©cÁ'§Jç?½Rô1Jèƒ?ÁEì6pz²?íßÍ°à̤?™°@˜B?'+6/Ì$?'äy ÒÓ?¨ížÖÛO´?•Å˜7h|?ípîfË°Ð?­ím±ùŠ'?¢)BûíÈc?¢ê±#e?¦Ç֗W*›?§ Xw¶à3FGL J0600.4-1934@l-1;â.^À3¼˜å>³šÀ9âÆo»y¾À;­1"́þ?ãٍ«d@®Ðǃ@r @§ºï¿è~u΅«ó¿é5Íí3J¿è&s†¬ÏN¿ïÿHÔ|¥UNASNone?îí2Iu?¯G×Ðs¢C?"¨‰'œD×?Š8ÿtïî?©G
tWy?¬×©:Z?åtsØùê'?Çíný%&?Æÿ§Î]?¿jð…ºo?Ã/-ôIúP?¼Ñ}
ï[?ë´M'<Û?¦ZÖå?­'Ž)ý6?–y³šJ?³–Laˆ?Ÿˆ_Hñc?ã‰/ß:¥®?³"%µ‹‰?É|@l¼c<?°J*iÎô
?È_Y?¯¥LÁÇâ[3FGL J0601.5+2309@gYW)²€ñ?ÂÀË6ʗhÀ9N˜0
À:íÒä>š?ÛËÆe!@—ñ5·ÇØ@àšüI½¿å²y3‰æ¿åKt­¸¿éc™Z¸¿ç€ †eéUNASNone?ÔJq<&}?ÈêÎû
zL?®	'<†?­VÃ7Y?ãøöÉüHú?ÊÔÖ
>‰ó?—ÈÌ«j1N?§¤°è÷?³¯ºe"U?´øðíöÑ;?ìËÂNcÄ?¹&¯eú•¬?ãzb_åL?¸žÈÃ.:x?·ü¿óžj?¤Îë¯ü˜?ÓCMÍy?¶.Cþžâ5?á—ɯþº1?¶—)ÿ.?°¿îîráÛ?¡Û–vµ?Ø päeÓ)?µ_ìgFo3FGL J0603.3+2042@g£ùHUÚ'¿æðí=…À:c–j:0}À;.LC¥q?¨âg-¢Ê@	ºRøöKv?÷ÿŠŸUÆ0¿ï|	›ÄC?ïqlÜÍ ¿µ/µz¸½R¿æb"¬
ÔCUNASNone?îsö¢†#ž?°Kþ}y«?kV yîèi?sßÃ9•?§3Ïþ× ?¯ÂƒuèÖ?Çh3Z§?ÐÁm[> ?Æ£ÓAr0ß?Ç_gwˆ
u?ä|þYŠ?ÒaÃ:?ëŠÃ6÷>K?¨$÷¦‡u?¡rʐb·?"ÙfÄ÷>É?ºð±é?¤ø±ðÞÐ?è×;—Ö׺?Ùnë'ß?°5ºÝÃy?¯%Õ
úg?ĈÃ5¿\?"eN¤¿3FGL J0605.0-0000@ió(àÉÙÓÀ$š¾'›þÀ9"àê'À;Xƒ°j?Í*™où@—8v,®@'T"¿Ò@C"OÇ¿âR€"ÁÆè¿Þ{>í¼¿ØèÛ8þ׿UNASNone?ïZAÔ?…ÕOÖ-^?`éO¦ñh?_;"¹-Z?‡ï%-aBq?"-0ŒËì?îorjúi?°|CnVŠ¦?zîdÅ>Ñ?'Z K+S?«Û<@­…?®Rk¦_x'?îoìü_?'~M´:Ñm?'¶7Á$H?˜ÞOɚì? 4²Ÿ§ì?‰N*ñ´?íïÒáǼ?˜¶c,îá?]49wˆ´Û?`î$ÒêÀ\?°˜ãü½?—ÓӒBv^3FGL J0605.9+2039c@g¯Þ¨—c¿Éß8IÈuûÀ8Àº;А§À:¤®á){?ô¶@K)t@cä¼Î@Þþ€N?ÎR	 pV¿äùóK'£×¿ë%Ʀˎè¿è6­Í>sUNASNone ?¬€OT tq?«ƒ†Çòú¥?ހBË~²?ι#zë2?Ýï×Ò°r¿?Ï<bxú?~l¨BÇ?•ðe§?Æ+š_­ù‰?Á¼µpÅm?ê8@ôI?ÂjÁ…"/Þ?κò¯†Ò?³¸lôøº?Î'_Uü?°ÓØËè?àË^üZµü?·Àhô
Uj?'úõçH?¬bQ>â?Ö§Ú&ž÷¸?ÁAÄ
Y[?à'íó
R?¾éË`r33FGL J0608.2-2306@l³­À˜$À3hOô4ãÀ:r(œ×;¼À;áàÈðŸ?àùµI^ª@
úp­½@štŒB¿ä´×Qyß¿ä@¦ñ›ä"¿ÌeÔ
È¿ïÿ£©	pŽUNASNone?ëh5jJ'?ÄÐ!%?¤ÃË¿š?¯ÍQ\ž¥?º»rɅÞp?Á#ði†±?é©Ø!áN?ØL.Ȫ?¹T'%a¨?»eä<?-?¹\¬qÒã?µ-¥«H.?êuªá>É?®ëår^à?·©Þs¹Ü)?¥=úUüQ±?·út5<-–?£ši¨â¯?ëÎ\åê±=?°-n©h?¡óõyï[o?¢•´‹§ßu?¸"²È[?©%Šý©33FGL J0608.6+5328@d	 {5*"@/›Oe™À:Ʋ˜¬À;œnCªy¼¿ë½ñwÑó¨@áÖÚAÕ@ðºà'$Ö¿µG㈿àŽæ•ÔF¿é¤Î#"¿ã'èd6¿UNASNone?ï¡	ûC?§vGh†?˜ñ&?
¨?¢ïýk=ò?xjá6†47?™Z
'üÂ?ï	ZWx!?¤9jܒ<?}©'nY;?…Àm·'?—jPº»?¡â›¯¡‡?ìPC¯¼Èz?¥<!õb5?¬¦)–õ®? ´*©(?$?®U›m>u§?˜k`ó÷?í¢¤Ò⋊?£;á³Ñd:?ƒ¾¼n¸7?‡SfxÞeµ?°sÛœÍ?¡Ë·½Ý 3FGL J0609.2+2051c@gµzáG®?âÎìóàÀ9-J´O(À:˜}–-ÔO¿ãoXš9Á@
n¹?!@.'`@3¿Ò1#"Øå_¿äÝ÷½l4¿ë°²@jºo¿Úð¼UNASNone0?·ÔÞ¨r¬Õ?»Èqµ²G?»ÝI0k-å?À¾.ž(?鉻äD¨?ÇÔq6DZC?°Ø.Œy®?°é–j©È?›€m—Ž>?¢ ¼=NVª?î6uÒßÁ?´Ià…á	±?ÒÀ)Bؖ?´_¨@9œx?ÂVÐæf?ªDý͌¨À?â
n7%?·$l™Éb?ábé$Ï?Äà(ì·Ö?|ÌY`ý‹?'2ÇP^3?ÜȼÈT2j?ÄÜ-åU›3FGL J0609.6-2851@mnµÇ͉‹À5/.ÌțÀ:J¥öŸ..À;æ,_Ú[+À"¦ÃMÈ@	A–xQö@ý`O¿èT-ĉ\`¿æZýñAѿ㜒i=u¿ïꆳ&Í8UNASNone?ïåá#LŠ?t÷ç\*o?ZžÌÏ®!?nÍQ#d_?[T!ì—<±?cøÚ0?ïˆifËPì?"}ö<À?h¤á ×õý?wÁԒ4pÇ?‡¼mäõǏ?Ž~žŸ˜sö?íÛTXšT'?˜6ãåd¼?ŸÑ >\þI?Œ†ð*@?¢aêW,>f?Ž¿Œ{ˆ˜?ïsc<ê]d?ŽUï€Ä)â?@X£×äd?Ve_ܤkN?'ÓCõ3E?zþiLƒ3FGL J0609.7-1841@l.ÄÑ¢À1bÑ9C­À9¢aÅíµ{À;›ÀoÇ88?ç	ů)×@~ÛËÃ7x@cËè ¿Ó;ùæ`q°¿å©O°´¿ç"Ky¯n¿æµêpLšUNASNone?ïÖ½­(?‰ýåIãƒ?'nkف¬?ƒÐ'ûÃÀ–?t7Ê÷Âè_?|#fʝyi?î£6iY?§³ðÎÔ?‡b=¾‡?‰VdNÕ? @׺ëÏ?£äꄱDŸ?îMþóÄ£ß?"œ¶¨&¼'?—Ølks#h?Š/õ ?h?žgµø`ª?†Ù©ËàP?ì8òs=?§5³÷mï?žÅ)ÚU¶å?'f®´ºhî?¸4íõÑ°X?¥îxcب3FGL J0611.5+1957@g×.œË}A?丝jßrÀ8Þ$ZR[íÀ:¾Dä5Ÿ?ôjÅ(=¶Å@³ÅPÉ@e@v'®¿ÂtÂvÔêö¿èvssârH¿æˆÅ(
,¡¿éœuʐUNASNone?"±GÌg]Ó?'¶¢5:ã?Õ>­õò?Íás"à×?äÛk"EÊ?ÎBItH:??êçض?žNxÛ1?¾ÿ?»¥Ì_zÞ\?ë3'@Ý?½Š$"&
?Кvzþi?²5jŽ¹T?ÎG¿¼9u³?±wMu(RW?à ÔÓr•^?·Äsš¹k<?ÅïO÷í?­­§Ñx¾i?ÑAU¬^?º
ˆóï|1?áãB9Õ°?¸$ó"0š3FGL J0619.4+2242@g¥Ô¿	•«@l'"øÀ8åtË"¾À:dX R…ß¿´j摏¢@Â]](O@ƒ 0w¿æsñœ÷¿àr¼‡Ò".¿ßNr\q¿äI͖ÑOUNASNone?Û¡ÿ2OÏ­?͝º°FÉ?‹ý‹}ÊI<?žZ¸«e?á¿
8àï?Íâ®NAQÇ?ë`"Q?Ä%¶––?'œµ0ø?‹¬4ewŽG?ÁUÔAP>¯?Ã\ے%šÝ?ۂ[ýÙx?¹'h"Á6£?²21ßhŽ²?—î
Ú(•?ßñX,(Û?¹ «ûÔ&?ã¿¢öÇç`?ij™G'Y?f²
ÔÁ?biö2m=?ØTz®l–?Ä©ÔëQã"3FGL J0623.1-4143@o1"…]¢sÀ6ªk\šÀ:…vWu1ÛÀ;âº5"¿ã¥®éjšÜ@©'#Sl9@R?'Kõ¿í^¤blÔ?Ï(²aøª¿äc•åHÞ¿è˜Ò?05UNASNone?ï™@MÁ?¡R¿œ'E?"jæW#LÈ?žbjl+d?'ƒã>w63?…{YÈo]0?î
'^@½?±õ'^w¯.?•:†r±£#?ŸÐ4\Rǟ?¤¹£ðÃ"£?©s Nš¥?ífcÐqÙ?œEž$_Q? FèuŸX?•©(ªOñ?©RÚélÏ?"±î‡Éò]?í¥!6ý·?¥Éîˆ1Á
?¡¹lþ!5? 'JL—Û'?£ôá#&m?™ ¨"Òƒ3FGL J0626.8+1743@hLœàuöý@
eä`gIÀ9;\Í`qÀ:~·îï6"?ôKg<O;§@&X¹Õy@˜Ëßçܞ¿ÛWÈ¿în…(jϤ¿çm+?Úò'¿ÄÒ*Þê aUNASNone?Áؑ1 R?Æà"†*0(?¥L2ÖÄ?ª˜ŒÃ…½2?ê5†+¶º?Éúõ[àõd?áÒâòž?Öáq'FÕp?¢(çj	Ž"?²ƒJ|OGÚ?ÚèÚ¨ô?ÕËö®)
¡?ÏHTŽ•¡/?·šTâÏûœ?ß«‰•Lã?§Ý‰	ŒÄ?ãEÿùõD{?ºª="5û?ßó6³}C–?È`BS¹?<<Èë?©þžpÚ£B?Þ9ô
s?È*omæ¼ÿ3FGL J0628.4+2429@g'^_0çÿ@ÔÃ\á'fÀ:û¥þ+êÀ;\nªƪ¿ÛLçDd@
ç݉Þe¦@¨‡Ÿqü¿Ýp_
ô¦¿Óø¬
ÿI¿æ=î"2	¿å‡†UNASNone?ì2)6Â8!?ºˆý¢5?š%řÈ×m?žÕ€ÑBÂ?·åDã|	?·SœVñø?ìÄ‰Ž¹'?ºÿ´Ï6È?'HRÑ$mh?‡eÄ}V½?¸ÈÑYe¦A?¹¤Çð7H?ëù˜!s-í?£q|r™!<?¦g£¦.˜?'﬇)±Á?´ÿm!O'Q?ž˜ê™âƉ?튑²:Ù?Ÿ¡Jg#?|(T"ûMJ?vm69¬"?±èí$é'ò?ž§P~­Êv3FGL J0630.2-0929c@kaЦv ïÀ!öúaZëÀ9¤,ŽÔCºÀ;5,)Bï?ò>»Õ-Ä^@!\q@ñgya¿k²ú•gC¿ìÒ
}¡/T¿âu	u…ÏI¿ïÿ'?¼UNASNone ?ØY
›?Ê	m~	
?ÐÀ$̹L?ÀÏÀ÷`}?ÝނՏÛ?Ìò
;\ŽÂ?Í°´¼"?Ì´4À€Â?Ôv‡§Ý°ß?ÆύÁ®)Y?ܱ1ÍGðÝ?ÉQ• @ø?ނƑÅo?µ#-5?Ó[²N/©?²¢!°»"?ÌC@Šî?®Ò>xŠ ?Óë«÷ó&}?µŠ¯²É?Ñ܊Tg\?½¦¶ÿ»s?Ú7ɳ¥}u?¹×ŕ[»"3FGL J0636.7+7115@añ~|áœ@8mDþ6Ò$À:
{À;ÑïSàQå¿øwƒ…*L@Ùº÷7Y‰@ڊ ,…Å¿êûRAsñG¿äNnU>¿ãš'"¼²p¿èèÎ̶IUNASNone?ïû€)ó4f?D+T
é¥X?&üAñC®?*ìÈ©Úk9?8€Úä)Š?@±UPZü?ïÈÒ/ˆvü?|ˆÁ¯:¡"?dqEZ"^ð?gÑ8uM\?q^EŽzÒf?w	Ÿ)#?ïk'"új?ìŠ›•¬¿?vE3‹[ÃË?p'òdد?Š{·ž?~
=ÿo?ïÓ¼ˆú?qÖ"Oá? †Hg ‹‹?+TÎÆ7f?uŽ2þ~÷?pØ1Uá3FGL J0638.4+5704@cÍ|ßýa@4ϋ&9O­À:Á=L'©À;íó?']<?Ö䟫›=¢@}'ûr|Ÿ@jÎ]=s¿ìN^·'ËA¿éÙQ®¯'¿Ë	àØ·*"¿ëH©2øUNASNone?ïòsbõš?·™$m[
?/ª×"¡
?7-Ò×9g?W#ß%bª ?µG‹÷úm?ïc9?.­7?"ê#ifò?'RÎ¥zõ?…ôXu®º?"ÞáH7?Š'}ÓoÖ?îõšñ l…?'å5b—H÷?‰À¹0¢é?ƒú'"¾¦?"ÀAZÉ?ŠñÊ'l??ï#t"/F?–«£vãŸ?qc	o°B?tp"·Ø)-?—8¸7Â+H?".{Aw…¹3FGL J0639.9+3250@fÁª:э&@(9äSÒÀ:
¬í#À;ˆðÔéÒÀw4x­Ç@6 \@ó@*·àŠ"¿ãÊ´p×ÐÙ¿æÍó3F‡¿é‡¤t>d¿ãžnÖRªUNASNone?ïÏ´[[û
?" #ã³­¼?`MîI¤Cä?Š‡ò•Ü3È?oý¶Z`²ƒ?'©‹båkû?î«­!¨üé?°8Zûª¿Z?nd`-#‡
?‹›è2¢q?£^çâøì?®ˆA"9~_?îE*¾CaC?™œ¨ªT?Hû›Í'G?~5°ˆÌu¥?¤[4և"?•×pùëÉ?ï½Éé]'š?|èãÞûa¹?	(nˆ‡{?$û"9#Ã?€t]:Ò ?|ά¸¡Ô%3FGL J0644.6+6035@ca…H©¼ý@6˜)à¤&À9¬Â7G"êÀ;߁SQ¶¬?­e±p›@eyþ§@63Ÿi½3¿ê…wßƶ¿à­¦t|¿àƒ¥p´À¿ÝŸôôÖx•UNASNone?ïçü5F~ø?i
p´¾‡?]—Ìßè'É?bÆD+o	Ã?Roȓ;?XùTrùd¡?ï¨-¿?›j?ƒkèï÷Hß?qðØa»ï
?pR.,g‰?yøGþv[¬?~:˺.(?ï*Šß¢=?Š€­*³¨[?†aýàa-?0bó³ßð?ŽûJXºu?€×"'êM?ïw»Œq?†OŽ~•$?^ڐŠ|z"?\ØKRÝ}Ê?ŽDæÿÍT¨?…VöZ73FGL J0647.6+0032@j€Îš,f¿ã"‰ÝŽæãÀ8›èPðÀ:ñ#±µð?ì­½Dõþ@.{ÏÚm@¨Ã ©-`¿ÚPâǜ'¿ê½"6± ¿çߕÒ9É¿âVxÄPÁ'UNASNone?àŒ+ºÝ8?ÇÂ"nŸ-?º¾\Ö%?¶ìù?Ê?Ø8VJÅ?ÈbÉÑ(¶ñ?kÝxýȓ?žÜ=²Õâ?¼Ùjugñ ?¼ÅÃÛné
?ëç#;o
ª?¾t"l4¾?â7j‰v??¶ÐD‡g2õ?¼!i}LƒG?£í'"¶c?ÔÏ6˙ò°?´¼ÓÀ€›Ù?ÜRb"¾1?³µv7«ø?¸W̒'?°}L%t?ݗª¸˜»l?µ€"•©ÛV3FGL J0647.8+1751@h'çÀn¹@˜Ôw¼À9Ži°ÂÀ;3è?ïÚ?óàÆ>hE@
»þ5¥~T@Ÿ\"¿ã†3é!ӿ죃äY9¿Ý<è7'¿äà劫6œUNASNone?Ô22û?Ë#nÚD~æ?³Á
A8T?³¶e2:>?ãnÎ:J®?͵­£è?åò8à*…¡?ÍU'po°?²»Dszçˆ?µ¸ŽêäÌ&?ÎÙzE˜u¸?ȟÝՓO?å$çÏ`;?±–ÄÌ*k±?Âcî­xD?¦Í¬²Ö?ÉrûH?«{n âp?átYÚxL?ÀxÈÍ?½[!Ñáý ?»žÞÖîÚV?ÕÁ&×Ґ?¼Î¬žMúž3FGL J0650.9+6524@bĆnCª@8s¸<òϖÀ:+gÔûoxÀ<µ¬õ–ðÀÛ²t†å@Ó,8Ã@R`E:¿ê£É²ªÑi¿ãd1_ô\^¿ãƒš"ÉÙ±¿ìH¹IY²›UNASNone?¢vöT?œ$P›­×?"¯%¬-mÕ?š}׫†?p^cl)ú™?xöûNÀb?狀9.¾?"Ùï¾+Ïl?j©©¸eµ?p­ÂÈ߁°? Î5Åü?'Å™äFy?íb¡xyKê? :;Ä~ë?¤ŠˆoÍö?"½Ý|Š¾?¥T]ïûs^?"l¡­3_u?ïÓ®[ïº?yØãLã‰t?+t»2^ô?HŒñå—è?uM .?y%"I€HÀ3FGL J0657.6-4701@p
:æ…ÛÀ2|?>pÎÀ:`%wˆÍ™À;µ£@âH_?äɝ¶gcD@
!¨[Ô<-@ÄÌ>?î3¦p¿áù¬_ç>¿Æxä ªV¿ê
%Á8L«UNASNone?îçÕW%)%?£ºSâ??'/¾‹?›'áªòÂ?ÕÇ]?Àø?•öchì0?ìâ¸ûã;×?º[ÈÙ,Ͳ?¤B"‡ý†?ªèä@äûõ?­'ܹÏ)?±«¶`?ëÄØbkJù?ª7Úd'¤
?²Ãv‡Œ?¢Ï÷èÐs8?®+¶<8B?š|
RÌM?é÷>`€c-?µ‹Žîáë?¢lþŠSå?¡0iÁ®ÑT?Ã{«>[ÞQ?³\Ó€:Ð3FGL J0658.8+2318@hÈÞ*Ã"@'äË:%•¼À:`e)O…À;¾eÌ³mÀtóL¾J@lõvº@ZË`6¿è‹á··ß!¿çOY ˜&¿å©MIg…©¿°ã€("lUNASNone?ïR°'"wú?¡al¹·3?cÂ]¹¼;?fŸAâ©V·?"1¤yÉ5? ÿ¦¬],?îòÅË3"P?¬WÀC6y©?gÅ£®É&µ?u!k?ž®'#´q?ª²œÚ&Щ?íðv†Eg?œƒµ5r[v?'Â÷ëœ?ðò6§Ò?¨–¸ë|?—ÛAUdÿ?ïà6¨hÕ?jG|SÑJi>ÖÎO³)(¶>ëҞyÇ܁?o¾–/½–o?jD%þ3FGL J0659.2-0439c@k>§æšÔ¿ÙWŒc¦¬À9-QîÊNÀ:ÙàU?Íu?ÖZãü>Ty@
Ïd9:‰>@3ÛËÍH¿å¯ÀCkSz¿åЬçef¿ägX6Lî¿çf.:ÙxUNASNone!?Ákä´r…?¾¿S¢Km?´
˜hȤ/?·£·¬˜(ã?é#SëùÎÙ?Ä©h' Ýâ?¢Oè©Ò¼?°>°CËv?ºÎìXËä?¼MÀ¿?넽v[æT?Á¸o¢ÑÎ?ßL]".¥õ?¹¾+¾Ù`?º[XœV#?¥éOVm?ÚÌE»Ó'?¹e¹¶?àä."=?¹"œ&WÎh?¥[NR™ð?"ÄU÷RÉ?ÝLÍáuhH?¹1³ §±¿3FGL J0700.6+3557@f™³=¯ø@1C'·þ	À:NGKîëÜÀ;Úa¶Ô=?åß*¯ø>@ÖшsW@9¾ Œ'u¿åˆ=^¸ÐŸ¿Ý°… à­!¿êð
-ð¿ïÿOÇF.UNASNone?é ôIZ&º?ÆH{ä\?Ê"¦Œ§µ©?Åâ@C{Å?…˜"Þú÷?Žð}]Éy?Ù«ÿ˜s3?Êٞº¥Éá?ßrsºÿé?ÊÆmwÊë?»‡á¶²3‰?·LÚªõ$?隣›KQ#?°å«®š~?ÁÊ$"ÿñ?®ãiEŒš4?¯-3ûNÝù?–sùcçÍ?Õ6×+>¡?º	}Æk¢?ã5®1¢?¾;å1B`?³E|•áxm?£JFq•ëì3FGL J0704.3-4828@p-xÔýó¶À1ô®…¹èÄÀ:áH2ŸÀ;Á™úèi¿ÐàF9Ó5@
¸ƒ«R?ÿ–Ÿ‹Á?äß5eù•>?Š9¼Ç?ÐƖ4èȉ¿éåH3ûUNASNone?ïFvvÃ,þ?™	a"ËœÒ?ƒ%íّ?ŠHñª'õ?‹<u:[/q?'wZYöP.?íOÇ⟜ ?»Vý'xC?¢1|¼ef?¯NîcØk?¨ÒÒIؑ?°|G˜²Õ?쁹‰¨ø?§HŸäª?¯¿—7Ãç?¢n‡Ði"ý?¨$ÉÎ8ºÄ?•lSRVw1?í0'+×!?±÷›Áê2n?†•ÞãÐ'?"Ç\@å$ö?³¬*Að?°êŸ"íŒÉ3FGL J0705.7-0006@jÕQ—¢H•@	Â?«ºÀ9ñ½V7D:À;Z³˜H`Â?êN¤d'•ˆ@ÛÛÐö¨@/² %ÏÈ?뗩Ás¿á0DZb–¬¿å·TѤ´¿ïÿ÷ç­£½UNASNone?åÆ$Ÿ·Ç+?Í$ªö³?ÒaÓ3Òª?̳Ů&"? eóh?©~7–8
³?Ô®w*œ?Ðæj7â2Î?Ç)¬t?Ãt_	V&ñ?ß¼¹ÿ©d?Ð?N/XÝà?äÚÔÃZ'^?²¾b]¥ø?̜cpû?®Ö1'"?¿ð"5Í?¥Ú
øí?à1(3b ?½fTÃ]$?Ñÿ'µ`¸?¼ëœã!ØÅ?Ë=<ãÞ?µ'ud]º3FGL J0707.5-3111@nVúñ€À%V"uÀ9Ïi,êCÖÀ;"ëžI+ÃÀ‡¹-2¾@Z±ƒED@±ù`~šæ¿ækMÿm'¿é|áp®úæ¿ç«Ø)2…¿Ú•2c¡ÝWUNASNone	?ï/HõE´ø?™ÇÁÑ9'h?oØF,F?r+¹0ÃP:?–6ß<@›Z?˜5È`f"?ïš;ð¤#?•
õ*¤?W§»ÅJ}Ï?iÖÈ}}çº?†|^Mê¼?"r­º:te?íkìBR‡Ý?ŸYEa±?—Ž¤Ëß?"Åxo?­yéÒMœ5?™Ab·é÷?ï㇨_.g?sØž	°>µFs5kª>ê¾¥íô÷•?lu®Òjë¦?sÕwyÔT3FGL J0707.7-1035c@l|"µÜÆ¿óñ'©"áÀ9/%Ž/LÀ:žYò»?í†ý1é@ÚHtñp@ôCÀI0Ë?èÞKb©î¿çÐgõ¿êû\˜1e¿éª{"œ UNASNone ?·"ëë'jû?¸ºN7Æo?Ø~#Ÿv?΢˦þ`§?àÎWð½÷?Ð7y¤?³úílǏ?ÀØHc?ÉìŽj†0?ŧÿ‰%ñß?ç<g.Ì{#?Ël£aŸ¿?Í£HØ¡&Ô?°o†¨Ü+Ÿ?Í?¾'ø?±ÆZÓæp?áG>)TxJ?µs-O…ø¥?ŀ(ðËü'?µ 8äDœf?ʎd³]†&?½Â'kbãf?ãü\–õŸR?ÀšKÒÐÍ«3FGL J0708.7+1747@hÙm›äÍu@'y»à~íÀ:d«Ï&CaÀ;·'ä™r,Àï a^ë@ÖúM8—÷?ýc8¢gI¿êD0¦2{ ¿è
¾Äî©c¿Èú‰ÏÞ5f¿¯P8ï—ÚUNASNone?ïõ¢{.?iwRߌÕ?§á"îO?'XIº ?S'fððcË?hÛÊ]P½›?ïjíHV¤?ªù®±"á–?d+œ‹?qWl|vÑ?œAãu
´?©Ý¶ærÏ?ïÙY¬¸Í?{mbBïÁ?whó(´çD?rÛSgÄäÔ?–ª˜;¬'?Åüˆ@(Ë?ïô"gS©?U"ü–ƒ>ð¢»Ž>ªM¢²œÛ?Wí÷¬BÖ
?U!zÞMºQ3FGL J0712.2-3806@o0¼¾aÏÿÀ)0HZåÀ9ÚÊ÷àÀ;uÕ`EK?êUVß	æ3@Oþáqõf@5SÀqt·¿äÆ1ò/K·¿äŠ‹ÅN0î¿åƒ¾`£Xà¿ïÿȏGÓvUNASNone?î99†?®'"ú5ì?¢Fƍ.փ?¥_Àܘ_?™.«¾q3?o	ûßõI?ë3Kí­ö?¾Eö°Œšk?­í[Z€¤R?©ç9%êL;?·nùÓR>'?µàL>8U?ëK*è3?ªqF6–?¶Ä	wÕ–?£FžUÏԗ?­ÅKB'ª?—2ù äš?ç!$µDÙ?°(
ô7©?¼ÁÊD^"?¦k€Xؗ_?Å*–Jûê?§F'à3FGL J0714.7-3924@o^ {5À)dBÇû¬´À9æxT¥sÂÀ;e?åë€@
}ŸVœïº@œÀ? ª¿Ç/I=O…"¿èšÿ'_I¿ì¶yš†åž?Ê•—R+UNASNone?êÊp(ò )?¾•Ì)å¾ã?µ£åôC‰?´™°¤ÅS?´	vÒz»6?µæ.ï«E?î–c€š=å?¶|¡ÆýN½?€ÙIç0¤?"w"žTÞ?¢ch#âU…?²ÛÑ]çÒe?ë;†@§ÆÖ?§QÇr"?­'Å°ÿ5f?š»
Fâ^?·Zë"B. ?¡.èƉÿ?ìñˤ¤ß5?²Ö¬0SE?'w–»«?"Šu§>?¶"°x0ò?±E<cä³µ3FGL J0716.0-4525@p
quŽÀ-âÏ d#–À:G8£µ|À;Á'²D‹JÀòõ¼Û5@
'1µY¾@åÔܑ¿ì;lÁnþ¿â2öà´¿åM‹\¦/e¿Ý"ÙgK#üUNASNone?ïӫՃ•?qýX³bª?Z&oe\Æ?\ˆ™m??o@òÉÜ7Z?nuŠPæÙ?ïÂJk˜Û?dí•.r?S'Ü¿2?aÚà3)]?yö=ƃŸ?}ªÅ,Bk"?íü	¾-Ý
?–b~Ӑ(Ã?–ˆW_d
4?†Ž2¨£±"?¤û8mp*H?e‡&åë°?ïÒÂX}ö?t?™/Uƒ>âÚpÄSo>õ)~L"ƒ³?ví戢´?tPƒz,3FGL J0718.9-5004@pUS÷ÎÙÀ0Vy_goÀ:¦ý/À;¡0-Å5)?ÈN‡Jj:@q¯åC;@"FÀXË¿äbîpFË'¿æeÔñ–¿Ü~;)vÆÜ¿íÊö´Ò°UNASNone?æå…ÜQžt?ɚSÍ'x ?³kµÈ<ãé?´š3§åŒ?Ê´
ª›??Æmƒ««"d?èݼ~ú?ĔVŸ¨
¥?»"ìŒ1·?¹*ίÐF?½ƒA/{þM?¹j"êZ"R?êô:Ξ0×?©¼¶5¶?±®à‡†ñ=?›qrlV?¶¯I‡ˆ?¢ìR_Ìæ?ç= |¶Ü?³åá›?°#g	®$?¤­D^ ìW?Êú1ù6?±^Tߊ‡3FGL J0721.5-0221@kOuŽ!–S@c)ÞÛhÀ:Pc–¨M'À;YeΑÀ¼Š`Á‹Ñ@
›ÔeÈ[Ï@w í?é¶æà/'N¿Ü.Êz¯k
¿áÜu‡t0²¿Øú•aˆºUNASNone?Î{+Ó?"ĬZe?T‡‡0/³?SiÑ«p`?"{4…<?ƒ¹$fÃÎ?î1¢®?¹~£‹šwâ?l%ó6Á¦ð?âšî‰RÏ?¬œ
²iØ?¸ø«ÈÏgd?í¨ª?ÚÀ"?šñØ;rxÛ?•öö²Â?ƒ§õÅfXM?ªyà»zçØ?–zÙ+	Œ?ï–'Ð&Ìq?…£†Î.ì?¾J܎Z·?q¸Bµ?ŠYM«pU[?…—èž¼23FGL J0722.2-2648@n9XbNÀˈ¡ú'+À9œÝÖ³ÖÀ;R¡w´l"¿ðóaHDg@
ˆÝrâJ¸@œÁ¿êPGÕpy)¿àՎL"¿å!ÙJåÀ¿ëÊ}^œåÌUNASNone	?àÚ±J©D»?Éw%Æ[Bd?Ó«w¸Å¥Y?Åë@µ~™¢?Å>KcÏ¢^?¾ÒRÍ@p³?ë~Ã5Мt?¿ä&—Ûb?–AaÜ#b?žÏxI¶?¾yÚvSƒ?»–ýÓi ¥?çuC,>3?°A6ÉIÎ?Â\ïwìÞ?§ÖüI½'?¿œ	[®4§?£;¤Vùùl?ìS…?0J?«,Ôlp›?~á'ûz'?‰†jàºÑ?½ƒå½ÖÆ
?ª‡Ëún3FGL J0725.4-5007@p\å@ÌxêÀ.ɶ'!%À:¼šTª|@À;ØúËÙ,?í+žMÒ@x³yi£]?ÿ€@W3¿á,s©£…‰¿ïÿ·¯'C?ïûûU˜°2¿Þ«úõ—UNASNone?ï´¹4o²‹?"¼Éc»ô'?TaÑ깶]?b\tnZH?€Ex¦¼&F?'äÉöݾ}?î•óÏÀ6?¸ËÓïð'"?ƒæ³'Æ0œ?™šmQ@s??¡§Žu?µOf`3?íÿC¯­?¡ñÓ¥°¬?ž[[Ø?!&Wéü‰?¯°r¾ý#?šï£AçÇb?í¶Ó??¸íAC™´?]þ^çóöž?'eÊP÷Zv?±×ïëØ+?¸E8vî3FGL J0725.7-0550@kÂW§†Â'@ªÄ°ž™À:&¸©õÀ;']<9A?çâÉ|œnò@äJ¾À¶?ý›ù?ò^W?êIHQŽ¤.?¢U'Õ«~¿¼Rk¡}'¿à)êÚ©Ú/UNASNone?ïÝ+3Ù?tœuºñ G?RrÿžV?VO†©äkÈ?i±ÇáüûÊ?qÞÅmÓD?ëö1éù"?°E¼¯Í—?l.ùã?š2
ðê?¼3e)±)Y?Á_û:O˜?îü
ù)7?˜z‡¡´k
?'œ5V.ñ?'»5$ÈC?¥r$˜BU?"úé&2s?í©Ø5•+,?¦"§s÷?ŽxÂïô®?æ×ÙTÌ?­ÄKê°)?£úXæƒæ3FGL J0725.8-3532@o`—ÌÀ"ôù;À À:zÑWv	À;qªt³0D?Ðx+úé@"9náŠ@ÞL€S¿éø$ÆLÄÄ¿æ7BÙ»À¿ãõr
É¿½céL&/UNASNone?ïKWðS?˜éDµâZ?qð4…æ`?~HÃŽ\>?'ôÔ"¹T?•ˆÜ72§¦?í)ìܛâ?¾$©ã*:R?‹†œkC|B?ž	Å²Þ?³Få²±h?¸ø˜bW0?ínrÊ;é?›yYÆȉ?—,ú@;•?'IãJ*T—?­'V?vá?–ÎÄNáŸ?í/æ7£—‡?¦[W³ÇY?pB("ê`I?zU<ÃU?µ|«¹¤Ã?¦ºÁ\3FGL J0725.8+0212@jÜÇ÷zö@@!U0H'ÄÀ9|DeNÀ;{àdYEì?Ä<fõÌ@õ½ê0àÉ@zDßØî¿å]àÛÍq¿â7ä¬M·¿âò|Ԛ¿ß8ÅJfUNASNone?ï3¡d(Ñ?¡œÛÛ8â?h–½4Ò¤?dWÚɆ¶C?š¦´,ùk?¡	{«ã"?íz
)U?²	¬:óúT?~ƒÌ É?~strkˆ¿?±3'}{L?±0@˜?íø–Ï,_?œ¤Ó×0?"…qÀ=h?"âc˜o?¦mPT_[T?–S¡oäu0?îBqYȚ\?"Zà¸:?p±Ä\Öfy?l¬-§pà•?©Â±×ۍj?'ï™d™Õ3FGL J0731.7-1914c@mRd"¿Æ·\"?ÅéÀ9©ÌíƒüÀ:ì±+†–ˆ?í{‡¬ ÷ @Ȭêˆõ@+ÿwD¿â%q/(rÌ¿í_ÇÑÃà¿ãöÛ¯yç¿×g£àeUNASNone!?Á¹€@^ÇÈ?Â9ÇA¾(¡?ŒìÈtdw4?†Î²fϚ?ëìμ1?Ã	Œ_þL÷?¢°G@`H?³º›Û\µ?°õªåMÂF?¸"üȈ?ì¶F/PC6?À2©Ñð?àvãàR?¹åÇ]hñ?¸§ˆЩ~?¢JPàa	?ØêrDü?¹›nùaÓ¨?ã'W(ô
(?»¼#Üsû?›	qå2ۑ? Ã=ˆRrœ?×,ºÄ½÷?»e6¸›3FGL J0731.8-3010@n†!ê5"À˜¬}¡ìNÀ:|"}ÙI³À;ÛeìÃã¿Ö•´2Þ4å@ÆËG;¨Î?úµ1 6ç¿ïÿ(Ÿ˜??ïÿ#üY¾¿ÚÒÁb$Q2?ÇñÎ?yδUNASNone?ïéêTx2®?föd?=
øÖÎ(u?;ÿh¹Ã¦H?btLló*?d¡
󞹃?ì·àŽæúŸ?ňŒ¨iÍÚ?ˆ9‡ó˜??ŸD‰CqØ_?·>Wɸ?Ã_F‡¨¸?îy y§¦?"c¨éÙ?ŠR[«q?|*[^»û?¡Ùaz×?'_2Ô| ?o#XnÓ?"‡"M»?G[ÑG•"?Uò¢0e<?~Wbٟ£ì?"qÒVIxÊ3FGL J0733.3+5904@c¿")³ú@<O…ô¡'À9ûçéóNÀ;ùŸ¸—‹¢?¹Q¥mü÷@=X´ÌûÇ@>2ÿ±¦¿ê
π8ï¿ë†ØÕÕÆ,¿Ó½ïù'j»¿èúÖ0´åUNASNone?ïö j/kó? )˯ú!>?QK›†D³? *KŒsŽÈ?#œ€×7?&°­¥e+?ﲞ½ãx|?'?ç\ÙIn?q¶X0WV?r\GùÜn™?u©ê¶j°?yji*Tì'?ïp6q®X?ƒ8"*<Þù?p™ë/$£O?q&Ÿ\ðME?‹¥n"'R?€ÓA•
St?ï§íÏ¢?ƒ
õ›?I{'˜à—?LƟGIâ?"mêÆ	"?'d+"÷03FGL J0737.8-8245@rq3|™®'À9t_ZÙjjÀ:
jÿR[À;§£@âH_¿ü5V¹u,'@
Üme35Œ?þµˆ€»®¿Ì4Xþ…Þ¿æ×(Œ¼¿Òð[Ç빿Åkí4²uoUNASNone?ïÚZ/+ÄÛ?y3ʕ­Á?*6ôy²ÿ5?3d;.Áð?r0ÆOúæ?x·ÿòá?ïǑJeMF?zžŒþÑ­?P&öƒõºû?U¿ûyÜ?x-,[î^?wwÚ6üp®?î½aÑjz¤?ƒÑ^Œ?‡,u×Ê?u®y6ÈXÃ?œ½wQu¿—?‡ÒaûÄ&?ïÀÍj¶ýÞ?wü"zéq>ѓž <¢\>êË<œ
s?"å¼ù·?w_ö"Ù3FGL J0739.8+1312@iÊsÕº²@0Ÿ(bõ˜žÀ:+ÈbÚÀ«À;µ¢4rÎ?ôT&£,ëF@¶½[À›@àpÍ¥»¿ãGÀ-#œ	¿é+œÔóž¿ïÿÁÄ[D¿á<ƒbê·UNASNone?í¨¬ök5c?³ß>^A|C?¥¢žõ·%?«Çq?€$?Ÿ¥#G+OK?§'2Õ?ëRÉ(Ù?Çe5EŽ²?·G3UsÁ8?ÁñáÝE?¬PLŠì&?´ÂÀî¦t?è8óX¢Ç?®ó¨_ÄE?Âv
Á¯'ö?¨ÒHr?¹LR	ܙá?¡.(ãî÷?Ý}º7†}/?ÊìÒÜ?ÙÌŲ´ny?ÐK¿tœÙ?Ák+Š(®?¹…ò–Yk%3FGL J0740.6-5230@p'DЩ*À,…æÿ}úÀ9ՓW`9&À;k¶1€¿ù‹·Shݺ@õÔȧÏ@×ß?k$ç¿èÄéeM¦k¿ßÙØ
e,¿æÊ^Eäv¿ØŠ—È<UNASNone?î9U‰ü?²'s	b¡?€bÐ0Ÿ=?ƒìÖðŽµ)?ª¥x^¦8y?²#,@V6R?類Ü:v\?‹¶£¬î¸O?^7ö[~ ?j7ô˜H´?'TÊ&ù%?‡ÜK'¡?íÝ:7 ?¡ñÌpX?Ÿa–"ùF?Œvìj>¬?¯AaOÅéd?œKMMË°?ï08Õ²fÕ?Ë
!̶?/:\x?8ïÇz:
?™ºÙ=>lq?±Ä¼ð
3FGL J0742.7-3110@nÆw[0À®S<½öpÀ9{lØÀ;Ød°ƒÁÀ0tY™#}@¯h¸Ñ@½üÂØØ¿à±s39¤x¿èê|ã!ð7¿ä¥ïÑ3º¿íŒì"Š³oUNASNone?Ú¯j:&+?Ç8æˆÅyu?¼Ç(5A<u?¸?N$þAå?Þ-ˆuŠ¸?ÈNtÈB¨ª?ì4‡b‹žD?Ådc*cÇõ?ˆ´Áÿqæ?Îê9öð¿?»E,É£¡?ÃòyL8?å*EÕæ?²0úÅU)?Ã	¼3?§E×ÎgU?ÈßN瞫o?¬$4üÑè|?ìŽ&;kåÇ?³¹tg]îe?KAá,¢Ð…?bk)Ô ?»XJbGŒ(?³­ˆhZË3FGL J0744.3+1715@i\í(Œç@3?¿¤Æ†À:0áþ99À;¼RÀ—4e?ìÝ$ݞÅí@šö†M@ៗµi¿ÓÝz:iïn¿âkዲ¿ê—Ž$"¿çAê%DªUNASNone?éØÔL‰N?ÃT?eè©ä?Æ0áòæÃÆ?ÂãE(ô[?"^f×  \?š€@On?åÜëÅv.´?͛𺡋Ä?πë(ëäx?Éãe+N?²˂vÁq?²Áž\WíF?ë|<Tð?©bQçn…?¶*h}Üÿð?£rŒD.üê?±I¶¨@X™?™0ЈƧW?×=°‹s4?À?ÃXi¶?ßùß%Y?ÅDmWCÄ?Áá¢žöæ?±~¶À43FGL J0746.4-0225@k¯\(õÃ@&*¯È°À9¦´%6nÀ;'ø
h9¿Ç*G@C¬@]XXܐ@Eß³.k¿ã¦H®¼ä¿Þý´7÷àn¿àjê.÷(¿Ôá)E\UNASNone?ïʆ[§*?'d¹¯§V?OBÚªçc¨?Káùü?wa|Ï~Á?'mԖê?îô'¶U?¢Œ°Cs{?o܇Ë]q?s¢J‹µ?ƒû\Ïɶ?¡XÿÀ_ì‰?îÜʎS{'?'ÕŸ(¿¤?†±Ñ¡	ôJ?~UTyR?™
Åe î?ŒP†¸#D×?ïsY\æÞ,?[hAZ?=Qt-䞘?A˜ýä̖?'Ž'l§ó?€ØA0؛¶3FGL J0747.4-0734@lF`ªdÂø@!£Ð|"µÝÀ9û™
þ`ÄÀ;wÖ	Œp¼?Ùý%	NÞ@fñ/
@笿'%¿ì+£3:Ê?©¸Á"bçº¿à›ƒ†²·"¿åë!²¾iïUNASNone?ï$ž@ö¢v?ýtýL)?}7IÂw?w8ò¶ ?"%jæ§?™»ú_}?éZv¿,%ú?Ä%´"ÇÈl?ªµ4€6?¨†>B«Ï;?Ãè×ãAâ?ÁšŠÂë3?í'À·ŒV? Ñ¥íc½­?–Xk\Å11?†'E'‡ˆ??«§¾ØØ`?›Yú¡ñÒ?éÔ `Rü?¯ƒˆÁõ‡?¶ìc‰®±é?¤¾—Ÿ÷Z?ºn™sÁ5?©mRÎAO3FGL J0747.5-4927@plçl‹C–À'ÎÛ0sÀ9ÛS¸
øçÀ;k(zrŒå¿Ð=tÄfæƒ@
pó'ß@B@0þ'î¿ç$
Ù©Ì¿ènè\ ¿ÓÞ d×ú¿Ý¨-óòðUNASNone?íÞnÛ^`Y?³®XYÂô?]ËR¾W?d"nY¡?°•[Ú æ?³hV»5_?ï7GíÂUÓ?™CÚÛ)+?lܹ
Ä?qqü~Ép?•{k$Sí?–ì"´s6o?ídñU$Ì?¡ºÌüˆÜó?"n—Ÿªi?Í«-¸/?°ônï?ž2äl•?íñ&÷÷éÙ?™ñڛA¤h?E¤Ÿ÷šX?MjXmç?°KQ}?™Þâƒ$õ3FGL J0748.7-5116@pˆ¥ÃÞç'À)1!îgQHÀ9Ê´øš°ñÀ;cÛêw¿¿áiô/3Á›@
ìŸÊ5BØ@÷L_ª	©¿Ù²öcm^¿ïs5Hم?ԡȕc1±¿æÇ"µ¦Y_UNASNone?îâ$Œ&G–?¥qŽÞ"±I?S¾é¯ÕxÁ?WÁÃÊ2¥?¡?¿ðÚß?¥2'äsÃ^?ï\:õýÈX?£§uV«Šv?h"ê´ˆãž?q.E±YS™?'féµØŽ?¢Y^2§Ùó?ì/4ò(
?¤=‹…P±?œ§Ìž…ï?Šs$ ?°®?·\eiØ?¡gØ:Fiâ?íê¦æÉ?®ø§\&'q?*¤"Ê!‰?@Ä¥­;Ã?°¢ ~äwu?®õ0‹—3FGL J0748.8-2208@máî¢
?ý¸Ž¼ÆÅLÀ9z
>GclÀ;0¿ö$µ¿ÜÞQêƒl@
q†,ÕK!@ìÝÀ$5¿è»q§{ô1¿é
!þÑ$¿Ø'ç5¦"¿ç†Ú6(UNASNone?éP«7KY?Étkс}?†BÆ9¨Š?ˆÚªj‡ñ?ÉY2%[8?ÉøíC×É?Ñ×øF¤(?ÓvaVz?¤þؔþF‹?®í€þõ'E?åÄS^?ÓFSl^?ê
†íŠ?®Ké	çk=?¤Ô®v&é?'Á#ÕîRù?"ÊFÀÃ?ª°-Í¿¬?ë…p'ˆÜ?®µ¸Û§å?fAÉÎ9?dFñðù6?Ìåö'£«?®¤Õ´.™3FGL J0749.0+4459@eÇ;÷'j@<ž†"ÄPÀ9áÀ¾¡ßÀ;âïÙAOV¿æ ž†~@KÃ Ô ~@ùY_í¦a¿æîÜü'.¹¿â^Ø܋ÂÓ¿â&(¦I€¿ëBýùóÿõUNASNone?ï×øH?u=]|â@?g¯UÂ
Ó´?e‰\>ô­"?aL²<­)U?lÂ魜ô?ï¶j(̈õ?€Šñ¿†Š?o\''Y#?n,Ki®Ž‰?ußQ'Ù3?yŽ‹µ¬]?îç¼äÙ¼?'íü=ï`?'ŠËã?ˆŒø,'w"?'Ý^Õ¸?Œ·þÿ|?ï¬HÓ¬È.?}S&â0Ôh?P©ì¯×HS?S 0O??'؍~Óf?{«é­w{í3FGL J0749.5+1320@iç×Ûôˆ@2Ññ{ؾsÀ9ñªÖÿµÀ;Ÿ»@³Nw?éÀž‡§ @ºd>@þ–Ÿ¿"•¿í¿úÙ{?¢Þ,1¿æãtS¹æk¿èfžàs¯UNASNone?ìÖþ4^$?·ojí{¯?µ²KéP?¶Døil·9?Œ®&z, ?';Ýô˜ä?ìŽÝÓ-ôá?µA6Ðp—‰?²sÙþj?¯vn×ď?¢å;òµ?¥Iã81?í,Å32Ã?¢ò÷ö HÜ?§?9g¦˜K?—Ü觮±@?¥ôse0‹?•ûÛÏ8þ®?æ"§ÐbyÏ?¶Òå»Ye÷?Ïɉ;›¯I?¶£Õa«cí?®¯^i¥ô?¡¶Âí'*.3FGL J0751.7-2944@n½ºˆ&ª¿÷‹?cÃÀ9u°}á­/À;Ù|¸[¿Í_:û ¾@¦H<Ú¦Õ@šÿà iB¿ÚÎmÝdZÚ¿énÞov¿ïÿç
)"f?ïþ¹ç܌UNASNone?îH­zbD?¯d2—>>?'ŠÛâ¶8î?˜¥àƒËIS?¢¯ºn¿^?©8`å<s?Ô¨>ö×j?Õ:‰ÀU‡¼?¥,D÷¨æ?³í`F?äY´•¼?Õ";äï(?ê­ÙÉOºì?«8Ÿ+Ò?¨Mta©	?–dJI®?¾jw"­a?¦¿š™'·Ó?ï}z¦"¬?•U¡'žÙ?"€º ?:HNõ½Â?7'+þI×?•R"çžt3FGL J0752.6-1629@mSýÉÄڐ@ôë?{@À9ÍRÿ" À;~%AØèd?ÝâDæ@
꟏&y@˜ÿ•!¿æÜ3"yl¿Ú ÎçG¿âm¡UrÅ¿çj;Çù ¸UNASNone?è/¥ò¯Âý?Äx1³éÕÉ?Ÿ
ðЁõ[?¡àõÔ?Ë`
0µb?òð`c{?çÏãY6,?ƞMbDá?¨mk
?¦ùÕ¼Dۄ?Ê¥+×M8Ë?ÄV€V{
™?ìCÔ¿F?¦kmšpãÜ?¢1"Í6ð?ÁGoX?´È•;luÂ?¡Yš*Ô?é°\}
‰?¥#7äx7?¯ «V
?˜ÿV"F̌?ÁwÇÍvF›?¢/&ÉÕB3FGL J0755.2-2633@ns-8Go*?ë©÷À9.wAýÀ;.ˆcp'?â)¾Fïu@(ä±ÅàJ@ÕÍØã\¿åÕIJ̬ì¿ç¯ ùN#é¿ë°ƒëÔÇ¿å['²ãÉUNASNone?íAô]íX?´è›Tƒ)?›Õ‰\V3?žŸWJ¢?­õù«ö!î?±'^w"ˆô?¤­òBM?°Äfú×=?®IZ‰nÝ2?­Fá"ð´p?ìÙ¯‡Yî?·å߄(ü?ë.[¾®Œ?©S•3o§Ÿ?§-DãM,?"½ÔRwOÙ?ºöRå?£åÀ½û0N?çaÊÂߢ<?®Ía­©tX?­Ñó­/?£Ø;ÁÖF?ËŒ÷¡‹Á?­ƒÍp)&×3FGL J0757.5-0536@l6BB…@'õŒÒ
ú/À9Á‡ŸœÀ;•úœé°2?ð»¼x@dV7o-	@LÀM£¿äECÃ'º¿él~_½'¿ìf;}{ù¿ïÿhÅ*/îUNASNone?çÙÝÂ?p?ÆÍaåÔ¹?Á9]ø7pw?Àk÷ÄÙ¸"?¾Å-!#'?¼VGÀ07?Á¨ 3)?Ä?BžN¾Ü?å['ß{y?Êø©ò?Éy9˜Nõ÷?Ä:{ù?æ#«•ýÝ?±•75æq?ÆHØ¿û-û?ªÎ~À…æƒ?Á*ô'¬Ú?£Üµ}$܂?¾Ç•Ÿ(õ´?¬n¯àõ…?è¢Ù'Må?¹%M+X\l?¼!žNgáË?¯wüiDk3FGL J0800.6-4806@pk"¦óõÀ"·öµšÀ9¤ØDЩÀ;^
œ;4‰¿æu«'	@fÚÄT®@|ž_Ñ÷¯¿êˆ5Nt	ñ¿æ"Hô‹¿èb"ˆª"¿ïÿ˜ÞL•ÊUNASNone	?ïõÉË ‰? HºÓ0ãÊ?wN…¯n3?†Í¿%)»E?€[K`&´?—Î÷4‡Å?ìQZï6ö?½+˜b?"i¯f^)`?šUf›¦O?¸ZÄî½ô?¸û_ñƒ?ì_{»¡*3?¤B"/Ädœ?­>'$!¨/?™i†©a.?¬É³!Ë´œ?—«íÉr^³?ëå8ìÂ`?¨ýÀÊL÷'?Œ€oËbp?Žn˜è{$?½S(‹ê€ª?§s@†G'3FGL J0802.3-5610@pÞ䣃'gÀ*YÛ©¢fÀ9ÏCŸ'À;w|ÚQ?ô —•Ž•@VϺ½Ö@í a´Ñ¿æ]†,n6Ù¿â:½h€Çç¿ë–‹¥|§¿îÝЮaZlUNASNone?žþak?â×?¡²:Ds?ícç`Þ8?µ+·۔$?ªBY<~k?±eýŸ
š?ªñïGFD?®Ÿ9¥«žé?胺ÜÍ?¿Ý`¸Ç&?Ç4™ý~B?»ÓÛÖð\u?Ð\"R=?²º•×WË?â9¦
?¶5årýFî?Æc¨•dçP?ª (+?¹ È8RÌX?¥¢'ô˜?锎³f ?´4JÚÏM¿?º:Á²þ«?«g!¶ó-ú3FGL J0802.3-0941@l½XdE#ö@%òéhSÀ9ŸúE«Û»À;ŽŸ±m¿ð·¹Ù&w@¤gÕ&b•@A¦`|l¿äÅMíHÃ=¿âøœ×Å+÷¿àРÖÇû¿ß×çõ"ŽUNASNone?ìQʨ;v0?»dFö.8ñ?"ÓãQ%Är?™Œ†JÔ?¸<±éÚÝc?¸óØâî?í±Š¬FjV?·ßÚ.AM?'Âœ+o¯?‹¨1±¡?°W^·s?µÐ»ÄÒä"?ìr´†~?§tV-M??ž™6øšm?ŠÑQ~'§1?´ÄŸ…u?£¦1™Ìœ?îFuIE…?š
¦$Ì?V	‹Þ½£š?XLBP"xç?ªècluº…?™Ô=qïaB3FGL J0810.5-5214@p±´êJŒÀ$L`Ÿ±À9NeÜÓ«
À;E"äE?Ù¹e'è
Ò@\¬ 7@f"_ ¤{¿æÃǞ`¿êÖ!"VˆÅ¿Ý•ôgµ4Ä¿çø¡¨ör§UNASNone?í÷K—mo?¾!àčV¹?q)@á [ ?vH®pÃç'?®f&ÊUÆ?½Ðg¯p|?ëŒ9£Ô+ù?Áßš"ýÑ?œ+Y^ÇÛz?¡%€u"Ê?¼"\‰¬©\?¾
þ8&¬?ìƒ&u:w?¤àg+õ»?›B¤Yøot?ŠÖWH;À?µ½µØj?¡qÐp8³?èb]Ae¯b?°‰xÁ"r?'¸ñI©ÎÛ?ˆ"ò£Zûn?Ì?lÑ4š?°Rα¨ß«3FGL J0813.5-0356@lG
Ø/×^@0C#À:ZPÀ;µ©FµÆ÷?æ4ô9´h@ÁìóˆÎE?ú¬_©÷¿ïû^Õ¸?ï­Z®CÂ?•ÉæÁ7¿ÖIWé9ÚUNASNone?ïõœ?gŒ}>²k?B2jÞHŽt?B´Ñ&kÍn?IÍF±GA=?f¾/&‰'õ?î󖹢å?£ÃZhX5?Šñ;!»BZ?UqØ Ñ?"‹:Å®ô?ŸÌ.`àñ²?ï¥üÏÅ?Œ[Êï;·¢?ˆB¦ïO4?€î'2­?"J
¨¾m?"™M.ä?î¤Cmž÷Z?£kñ•r·Í?•–Ùd?š–v>©ö ?•à¸è
 ?›Bq§iú÷3FGL J0816.1-5044@p¤´êJŒÀ!9¨Íê>À9«aB:7À;#þT.U~?ôŸY÷î
º@=FŸ¡›q@òÙ æ[¿á‰3hH¿çNM;®=&¿é
ÂØŒ[¿í'íõUFUNASNone?«¹n"Ø?©ü'lq?áóŸwD?ËÜ|8f'?Úfìfö?Ë0¢ƒÞÊH?½DzÚ{y?¾åŽhÙ?à
Ó!§ç¡?ǦBlx?بçÏù'ß?ÅOÇ.t÷~?ÙωÏ°™?²¹½Á—e?׿Ls¶Ü¸?²bšíêè?ÌâSzˆå_?¬-5Åë?ÁsI;·õ`?¦îæP³¼?âjÕ''z?»`(´k?Òr·Ôâ\?µH¯ç3»`3FGL J0818.0+3237@g²(¡ß¹9@?WG²JÀ:8CÔk&ÀÀ;çÖNUο©¢ñ^¶öu@!¹f"‡Ý@q]À¥w?ç:¡f—Ž§¿é©a¿Õ$¾í!g?¿èaFNm÷)UNASNone?ïðHøàÝ7?ymúôEŸ?1Z`:1EM?1°QF?v«?[v/¹??yLÛ7Õ/?ï›ð$ês?…7'½¡¸?wã\<?u"^	œü2?zì䧰#F?‹ž 0ç?ïù
Aï?ŽIp%ŠáÊ?…QB?|@i«cG'?" 4½T3?‡ºÌªu^?îü˜?}Œƒ?˜Ø^Lr<?eߌ§cŒÉ?d¦Æê'è?±{aýå?—08î	P[3FGL J0823.3-4205c@p<†DR?hÀâøæ0K!À9‹j˜û)À:»Þzt¿ñŽ;AŸˆ@NûÆ_u[@~µÀ@ÍP¿èBS¿âÕ­›rü¿æ¹Lé×cm¿Ðõ›Ã?…QUNASNone ?è·ã{<s)?Å°øíåä?"¥[m_;?—bY0iäK?ʋÑÇ ‡w?ÅZU. Nø?ëF"nõ /?ʒ2
Ì ¹?ˆ âäõŽ)?¤cWÇ?a%?Ác¤Ü&_?ÈÌ,aa,?ã©Äè?0?¹îý`ªJ?·º%…vf?¤µÜeÏx`?ÒêìÎ$?¶ÕXiûê?í1¾bDu?°WxÖUkÔ?b¦ß[@ö?*ƒŸÓwÅ?¶j4D$€;?°U1°…'3FGL J0823.6-4838@p"HýŸÓoÀ´]+TBÀ8ö$"]?vÀ:ó¸°¶Ñ?õAš	.Ï@þdRåÖ@æW_¸Lb¿à«l	¾o½¿ëÝüÓm®¿è8¢ÆœS¿íOÂNÞNUNASNone?ëço1÷óì?¾`]ÍB?ƒq -++?†ùÕqëá?¾bL:»5?½¼Ã¶²4?⏠/O¦?δÿÙ ^?´ÂÕ˜Õ?²SUá™Þ?Õ°
`ÍY=?Éj3';?æ|ª²Iq?´Õ«"ô^µ?¾×šÏ¢Î?¦ª×Vôë?Æ¡‡Ï
{8?±=AƒÍ¡?ãt¼"wÂH?¶ÏÔJ¨Õ5?¸Î²Æj[h?¬Ú1óô[?ÒâÛ	uä–?´¥læ×/…3FGL J0826.3-5056@pµìß&k¥À…ñ¾ôœõÀ9C¾b¦¾EÀ;*Aç+ä?ð¥YEÁ€=@a…'ͼ@ÓÖÀk•z¿æo0m
Ó¿È©ü¯#Õ®¿á¡Ôñα¿ïþCj–fUNASNone?ÒCæêI•®?È3ƒ›:‹?â¾ô«¥Ü?Í;´ÆF!Ï?À|_|Õdq?¿_7ÍÉ5»?À[QCÖwv?€=¸Rªú?à1Ò,™?È\Õñšº?ÖÓó¹¼½?ƿօØ?­?Ú	‹`œw?·fME…?ÚYQØ/ÅÒ?¶8v.äy©?Ç:Y8ß;n?©æJ|Ñò?Ól'Ïd=f?¸¶…½aì)?ޙd×óš*?À·ìút\¦?Ëô±PPÞ?µ˜SK
O83FGL J0826.3-6400@qfþ=ÁÀ-L4"…ƒÀ9õVI¸±À;­i#L5¿÷'Ìg¢%¯@…×Sƒ¶@¼tÿ[j_¿èš¨
ܹ¿âs? (ÿÔ¿ê#2X(c¿Òpå;¿¯êUNASNone?î=«0Û3?¨
æuA\A?—"Õiäê? ¾K±6T¶?–Äu/ÿÖ? °PÂÚ?›|M?™f^:Ö?hFãÒ!?M¨ÓÏÝî?‡ùG¬g=?"§O{q¾Á?í-BSÌ ? b›nãßÊ?ž½£~²ƒ?Œjoæ?­Í	Éôb?™‰õíYB?ï#C^n?¤?'P—¤þß?:¥¼´g±?Gl$¦#¤!?›,ý?flÄ?'?2SM?3FGL J0829.8-5239@pіœ#·•ÀªB9`tÀ9rƔ¤gSÀ;:?wTW?×Ú+´RœI@
€ˆ!ö@}úÿåþÍ¿åöR­!¿ë½²8Ýþ4¿â5Ài;'¿èiÕ°ïUNASNone?ޚunyF?ÑZºÅ-?…ýa™$çÙ?Š'€¤Ç2â?àZÏÂL¯¾?ÑQ
SâÎÒ?äµ56Eóš?Íy¿¯'ý?±Ö%[-×?°Ìfçý'?Ò 
MX?ȖcY·_?êà"b?¬ËL0}î–?¨Z†öH·?'Amú "V?ÁÌi	ì\H?¨µ7ø!ä†?äò²b>Ã?±˜ä[PìŒ?¡¥"¨D¾?"9ráºÄž?Óåè¦pÛá?±gyNý3FGL J0830.5-4452@plÎp:ûÀ
Nb®•ªÀ9ò"Ýr6À:0‰ÁµA–¿ãö¸%^
@‰ÿÈ¢œ?ÿ9{ßto>¿éP¥:üD#?ï½jòŸd?Óa°¦Ûj¿èF¶]I²&UNASNone?Èiyù¨s?ǺsÏó½? –š*ˆ–?¦'ô
̪?èÜ^GÞíZ?É°Ddöfž?ê´h*^Œã?ÌÛz}S=?™4Ž
òö?°ñún?Áú¸ÄÄ?ÉÁW\!Ï?Õñm4@s?²"†›Š}M?º×P¦S®¸?¨É=ÙÀˆ?ᬆ4›ið?´GÐјÇ?é‰X©Âm?Ê2â±0ii?fóEh$Òb?|a¿¯ƒ?É~Ðã¸c?Ê7"ûz­ú3FGL J0830.8+2629@h­>À//˜@@F¾œˆacÀ:-Ü^:GúÀ;Ê zÉʺ¿ÒŽAX²@&@HNx^@tPÿ÷Çw¿ækš
+í¿é*l{¥¿ÜrWÙcg¿ïÿᘴ(UNASNone?ï㱁;…?tøÓvF?E—g()§?H­øÒÑ݉?gž¨¤úp/?sµ"¶Ÿ˜)?ïRl"¤UL?ÅFÐ3®ß?†£Ñ]Ã?'áÉʕÓÜ?"Á
΍'B?†šíþÖu?"™Sf?'ß—æ:þ™?"§TJ?…t¡¸¡?˜æ»ZFÊ?‹t!ONn†?î­¹ÊnÕº?–=Õ}j?{
?zCü¼2·?¡Âaµr¡Z?"»X™ý{å3FGL J0832.8-4321@p]1¤½º
ÀzMÙ§¦£À8ßÕùµcÀ:p•âTô?çžR@i§Ž@¾½Òß@`•ì翌»Ë'%Þ¿êFÑËå¿éô{Kû¬¿ØBR'X"¦UNASNone?º¤¹¸8 ü?¹<Ù»ñÆ2?Á'Iý>ˆ«?¿鍤@?èJÖI©I¶?È+=?ÖqK˜u«?і)8~¯K?µEŪnZw?·é†Iâm?âK¤åùÜ?ÐýcD-?ÎJäª.y?´¸YE²º?³ ß ÿ5?¬€°üú÷ó?ãÀ^Œ?"?¹v!0`b?՜¡¡Bº5?ÁÀæ¹® ?š'ü›Pݎ?þ‹§^2?ä]J"ù?ÁãÑRêÒQ3FGL J0834.5-4825@p¡JB®Ñ9ÀV¿2/'À9hhó ¸À:Äþí±Hã¿Âï÷<j
@Áe¥÷ @€w´—¿çŸÊR@Œ¿ê¤€HBl•¿ÞŠz܃èÇ¿êl¹oUUNASNone?àç¼0-?Í{CJæí?"Š¢Àö?– i#w?ÜçӞU?Íà`«'È»?ëWÙ»Á=?ÁëÕÁbÈý?íôø]ò'?™«=¿?À'Úqî¸?À™Ez%úÅ?ᚠ*x6?¹æ±úË3?µü8Þkôº?¡B"Ùßü?×K±t*d?¸w`Ú¹'I?悪¦›ée?¿.†\íÎ?gÿ+ßæjü?cX<¹M™¬?Òʬ[``?¾ê¼ºÃ÷Ç3FGL J0834.6+6101@cpŠGìþ›@AõÑN;Í6À:'dgˆ¥VÀ<
n.±Ä3?Ғf)T¸@Ëg!wI
@S;ÝÛ¾¿ÝpÑF⛿äpÓàx"¿ê'ÃC-ž–¿ãM®23ËUNASNone?î¬'YœJ¼?±¾-¦¥Ì3?¢uƒäOË?±Œ­/p¾ê?vCï¸#¸?vx5-¨`Î?îE,"5µ?­Q¥‡ž?¡®t
RSX?¦6'¬+´?"ý‡b4¢¦?˜zD¥º?í5Óe&'Å?¡"&*ýT>?¤Èd`j[?šâ༅ó?§ÚeM,ˆ¢?'Þ[iWÿu?êü¦Ëؽ?³_&c?¹
gu'3?±®=À¤âŸ?®ÄWYÝ-?£7Î{A+B3FGL J0838.8-2829@oS\gßã*@4~êÁªÀ9©Û0=À;r-͘¤§?òMÂÎq<®@â†óNÂ@ÌÞࠔ5¿àth‡©¿àƒ÷à"¿äŒÌV°;¿îG\sQUNASNone?;|óT³?Š¾·ef¶?ëUŸýŸZ?¼8˜öjk?ÀµÈ:JR?»ûfŸô^?¦|2Ö'ža?ªn…‰DŒ?äˆç\¶?Èï2($O?Õ
gց -?Ȇ…
EIC?ÎSlu£#?²2‡²N¥&?âÅÇxM?¶]XÓ9À?ƕϲVh?§!.úÛJ?ÉX=]lÖÎ?®AN›U?å¨Mì!î?µó%1$c?•!jâ¡?«-fGsV13FGL J0838.9-4056c@pI*â—9m?Ó@¦¹<ÍÀ8Ð/9©núÀ:mSB3'?Ä\G‹|Aç@Ù@ºZYh@MüŸù/+¿ç×{ÉÇV¿é' ÚE¿ë³3§*¿æâÓUÁÂFUNASNone(?ᓤ£Fþ?Í9¢%È$?²ðéiò?²†jáÓĖ?ØXz²·©€?Í·-Døø_?»0³h§e‰?ĘÿšIT›?±Zú—zÀ­?¸ïJÕ.o?ênŠ?û»9?ÉèDÄ×q?Ó¿ySn?¶.ì—?È–C
,?¯&¹½6+?àÙÀ…¶~?¸;`<·??ٚ~_ˆÀ`?Ãr0¸ÖƒÔ?•¿ÅS)'0?\ìéœkÔ?â"Â¥¢V—?Ãcá5¿3FGL J0843.4+6713@by•$Ý@A͂¡ ÏÀ9¦sŠ;WÅÀ;Βßk5?çÌ'æs@uÞ©n#?ÿàß=Ù¿æÑ´¬ß5¿Ü¬È$òRÿҜz¿;Ù¿ìº9$
üBUNASNone?ì^‰…Øyô?º‹â/wî?»QÆY'Îm?¹ß¤­êõ?{ž×z–³?Æõ¨Ìü?è4SŽùÃÛ?Ŝnzi?ȇ€"šÉI?ÃY°'â$?ªœÄ½ø1?©,##fœ?è<þpl®?²&Vî-˜;?ǏËXä?°Ÿ†íöl?­ô
Ëь?šÈ:xôQÒ?ë¨7?%Á?±*¦µŽï?³+ƃ,VJ?¬;i•
?¯$ÿ¤÷]?¡Ü!ƹs‹3FGL J0844.3-4741@p§Î_oÒÀ¯ŠúšeqÀ9
£oÜ0îÀ:œÖÒ	L°?ì%p|ê·@H©}è88@±>ÿo6o?ïÿ¡"uÿr¿æ%ºÃϑè¿çŸd}G¿ìZíß
Ž€UNASNone?ßÕÊÁ9‰?ԃ'RË?Ù4ä×¾´?Óo SÐx?¾év§?Ä4Mû÷To?ή¨qàÃE?În\³eÇ?ÏàÎX¨?Å÷1Õ2˜o?à\"M]®í?Íx»xOG?Ê3WH‹GR?°M–÷GF¥?Ӈ<¢Ü+?²˜šg
å?ß_¹´€,?µ¡Ð¯¶è;?Ä|õ(c>í?³x	ü@:n?Î1è9"ÚŽ?½ÊLß:g?ãTH§…ù¢?Àå¾fnÕ3FGL J0846.8-2638@oFÅCk›@$ªkøvžÃÀ:–ç7²À;œ}>ïÿØ?˜ÌÖõÕ@Ð3f´¿æ@ÈX *,y¿Ý´…XDοëX
Ò?l@¿ïÿ™]-š?ïü…û4Ç»UNASNone?îÎ(ìœT?¬ca'žõ?x{^n¼ðß?ƒ"æŸ}pâ? Ñ£^œŸ?ªž
'ié?í¼§Ï€Ë?¾Ê2gPoø?'Íÿ(ÔÙg?›IW×´0?¯'=Èìþ?»%ˆÌý
–?ì(vŸÁ?£J8 Åú±?¢ó¬[Ä?'Xœ@§Ã?µ»
y'Ô? ~ —baÃ?[0Î?–?µnˆö??B†»ø¥?b¡ï¸žW?Ž:¨k`»?–B`§©3FGL J0847.2-6936@qÆð:û~'À0@ ÇÀ:Å~#òNÀ;¹ë˕•(¿õ¾"_¦XÅ@™ýAµ@4÷ 2z|¿êu)6Òqt¿äëE
¡¿¿ë	õûÖ`Û?±zG(ÒiìUNASNone	?ïãlâ6ÁQ?rŸzfµUZ?[KAۉRl?hGŠl?]Úù¶ô¤?c÷ºô¸
…?ïÃ%¡Dæ^?~óáJ
§?Sh!݅?[hó±Ë±Ë?y"+ÄYx?{<F]ØC?î»zà'¿á?bõsyý?‹ëƒ€}§t?|Réãñ?ššâ-‰0)?…°ïw	:?ïÕ?Äë•ô?rBäÖ¼°>ù£¬¥Û?éÒB'ê=?uGç-Y;?r?nóý"à3FGL J0848.2-4524@p'3]$žE¿ò.Ñõ*¹èÀ8Z¥öŸ..À:AJFu/W?Ü[wµn6i@*°ÁÔKF@:3q¿ãΞÜØ¿è‡Î¥%O¿çÚ¸'›¿æðu̓tšUNASNone?¤í_;	TÙ?£MvÊüÝ?¯_	
Â2?²«]®y{–?ì»9|NŽ?¶ØÂ@·–?Â~­•j©?Ź*'n+?À€æïÈÎ?ÁôÍÝ¥è?ç@Þ³"?ËZRëBj?ÅøžTu?®\¤'1òÙ?ʓcܯ|I?´tÉO¢¹\?ãÝ!hl‹Ñ?¸W&ñ^?Ójnš;?¿ôC9‡M?—"›˜Í¥¥?‹;¡Æ[)‰?呴luL?¿@ëâg§£3FGL J0848.5+7018@brGE8ï@A•"Ý—ö+À:€€VÒt¬À<i[
lÐÀ‰©6šœ@ýïÀí›y@eÀy,g?ÏM¤È½|¿å[¦‡ÙL¿Ö0«±LO¿ãl¥‹«UNASNone?ïüºŠ£Žø?@L4}ëó? †9@ƒ?9k¬ºC«ˆ?2g›ë§s?1ÙJ|'ð'?ïÐs§Ä°?{šl®ŠI6?bR¿äwj?f­<ÓåP¥?m9²sÄ=¼?vï¬
"›?ïd¤5Ó¿??'E"~ è?~pûÐá‹?yuE÷s™?‡žt¢Ÿj¨?vžâAÖw?ïíGͪŽÃ?e('²Êš1>Ün¡iJ€>ð¸Íá¤$m?b©ûR ‰X?e q'úDP3FGL J0854.4-4404@pŒîËûµ?âRuÚÀ8"­¨DWHÀ:DUFƒr?êOI£Ú\¥@¤'šG@Íù ?{¿âªÙ-5ö»¿ê"¶Êh*¿ëÅýÅ_'"¿×1¼áUNASNone?¥¼ƒï͈†?ªûu
^k®?°0Ù-‡ÓÂ?¶ü–'0J*?ìž›R,ÿ?¾R+`&Œ?°£ö
Éw?¾Ü_£Ø¡?©‰ÁÁþûÑ?¯ºYN^8q?ìRå"&áb?Áh¶ž÷à ?Æ%'Þóý?¬ìù-wÅ°?Ì5N7F®?¶U)ÅMú?ãiGúqU4?¹Ü8¹x¹?ؤLë2Ðò?ÄN×µN±?—–L5Aàr?ÄI(`#e?âñ'(¼ˆƒ?Ä?º¢6U3FGL J0855.4+7142@aÄû~ÿ—@Aœà\̉±À9²õÚPÀ;¾½Žkh.?Ê*êdbU5@_ÝË¢«;@"5`4>¿âÙ±8¿æËÜ2¬‹Ë¿æÆCG¿ïÿêaïD'UNASNone?ïÅu©D{i?·|Ñç!?SÞ~&œ–?|$rðÖ,u?xM‹¹ø¤X?‹t•ç†MA?îö9ez×?—*yõMx?"7Qa÷Ö?o¢nP-û?Œ
ûÝZÇ?Œ½½™SãE?onî?˜ã҄F²\?÷ãªFö?‡jÏsÉ>?™UO <þÃ?"ùÊÖ_?í±<,Lq?¢<O«½›? ³ËÓ·?–PZÛ•¸?¤Ñ‰ojÑå?™|3"1J"3FGL J0856.4+6429@bÔ_Eà´á@BÏ …±…IÀ:wÖ²ÿœ-À;þ¿:=°¿£	ëû·@±¯ØuLˆ@iƒÿÔa¿ê_]Zùö§¿áÎÂ7óaa¿ã=ÞNn;â¿âˀR[þ•UNASNone?ïìsãÜJô? 
ÒÖë28?Zûý†¡i‡? 2ïµÒj?H8u'_u?Nã½n<E?ÓàØ5?‰ó0iN?xëñª=¶?µÉº ¸?yˇé§ï?|Ãø¤…jÞ?îë'°Ž?"ŠY©Ä?ˆtŽ¯2A?}¨'b7?–bø½ÒU?"Û â-Îö?ïpÆÓÜrâ?†ù ù–{?m+Opu`?gÝ:4¼™B?Œƒw,Æ›?"ý2j±43FGL J0858.0-4834@pÊÅXd¿þc@A8¯À8÷0t<ÿÀ:T¹¼NÐH?ðjÓ*‰ìR@
âjé,)@•ô@")›¿é¬p®i¿Þå;j܏/¿ízíBIb¿æ#}"ÔÕIUNASNone?žBôšR?¥<ѧQ/?áxï‰WA0?Ñáë8ÿ=$?Û-<¾3ú?ÑÒg$™è?ÇY?äˆè
?Êôèz|"?ÎôöFðå–?ÉI–Ür0M?âlru!Œ˜?ÏBÌcËì?Ɂ£ð³E5?®Õ2ð÷.?Ó\°×?µìEàû´?ßâ¬VÏ\c?¶ƒ¾Þ"qš?Å\kUـÆ?»D]è?É&÷÷?ˆL?¿D'=ýÔ÷?ä_',¹½¼?Âû"Œm23FGL J0859.3-4732@pÀ
»Då¿ð¸±§­X"À8±öFBÚpÀ:J­wœï?ëñ&D§Ã@
2L["e†@^¡`^x?š¢öÛ+C׿ërò·~B6¿ârKuãö¤¿êM|œÖUNASNone?vâFwq-t?ƒ}#«oè›?Á.bo4ý?Ä£‹•1åº?놢˵Pf?Äê=ž©´ã?›('¢†?©ÙV½^Á?ÍÆþcÚ?Æ;yùÄè?ç´üR,½J?ÇZ­a´Òõ?¿••U"V?£ñŒ±rAl?Ë¡ñ%^"?±٘À?å4±ý¨Ñ?²Ú"+c}?·é¹tdö?°‰}ç˜{?´€2ž¥Ï?¦ "·b?â?ê'xË—‡?·Qh}ֈ3FGL J0900.0+6754@bL"‰a=@Buk¹Œ~(À:ùÂÏ	À<´æüù»?Чɧ‡@©(ÃBµ\@è¶à|W¿Û|õĒÁŽ¿ä7æN†©[¿ÜÉnûØ b¿ïÿ™äOUNASNone?î¦Ù#'Ž?¨©Pc÷
÷?žÝ×°U?¦¦ÌMùV?Š?•ûoûÛ?‰¿òrozÁ?íÁR.…?¯ªçS%I?°U7¢	<?§ÛôUÅ?ÿ¿2
|?]8'5?뒢ºo,–?ªYÀ~í?¶n¿þó&Ð?¥Q1ó˜uv?©øT[&èü?—ý»N°Ö?í`O…,Û?¤n9Iw"r?¦i"<ì?0Ùàı?£îéFiõ`?—ŒNÄ\Ç3FGL J0901.0-6725@q·}'ÔÀ+ˆ}€^_1À:D!BoçÀ;ºÉ«¿ñ0Ìxéö©@
AK<>u@0ـ9vC¿æS÷'.|{¿åƒéY€ú¿è-h+•¿äGïç?PUNASNone?ïaäómo9?œ'ôز؛?g=:°`+Â?kØ-DÌy?Ûº<F~?šJdü·o?ïk?FÄê%?›È8C—6J?n'ý8ì®?WG•·¯s?oŠK'?•Ë¢U?í¼–q®'?˜PÓv2‹ª?•éŽ«1nø?'¯£"Þ‹U?©IÿCL_o?"x§—÷f?îéÆQº¼?'ÏG!š!
?QÖÅe~ö?S¤˜'9d? ÔäÆ9(G?'˜…Oý%3FGL J0903.0-4826@pÑXDЩ¿òÛç‡c60À8ÓÝËø'wÀ:Y8Ëùh6?õ(Ve½I!@
3´k×êb@¼2@·?ê?sÃq.k¿êIˆÆÒP´¿èLd¤LD¿ïÿæ
æÀUNASNone?…DéܺÅ?•$ژüÙ?Áµj;Ð?Åz<T]Ÿ?ë='Ìä­"?Æ@¶óœ?gÁ&UËäÉ?ƒúQùW?à¢VFìY"?ΊOBÊ2?ދÑ%{µó?ÎÅg'$?²Þ™)/!Ï?Ÿz=ùàëx?Óðä#+ùf?³ü‹3?㫺ÉD?µ5Î	…êÉ?šluÿÙ?'À·0Ø´X?Ü-¬GÏ?ÄDtX!9?áyに?ÄMîõþø3FGL J0903.2-4744@pÉAÝ!ê¿åߑ€EŠ¤À8­XIm1\À:\ƒ‹:[F?óšzí±ô¯@Å·n–¶@Aäpb¿ìˆÎñÅ+?Ð$fJÑyI¿éKÉ®¤Ÿ¿ç;ý8>N´UNASNone?ÐüžíDá?Ƶ28"¯?ÝÃý†ô¬¤?ÎÛï2V¶?Ñ?èÚz?ɺˆú¼µá?ÅkÁV³±Ë?˅ôáé?ÐO‰´CZ?ʖœ#b½J?â•çåxñà?Ñq[…
î?Ð/ç2îP?²d'úp`ì?қEr¸u4?´ÍÿÓbSi?Ý5±¦œ{?¶rsÐNg#?ԍX^žþ?ÂJÛŒÒg?Õ¯¿¤Ç=Ò?Â{"NÌåº?ÕÂçüšÀ1?½IÉë3FGL J0905.8-2127@o'>E@0òædM‡rÀ9›†g­ÓÀ;}´{/P?ó6Qbô@xè±Ú®@G—¸òпàÍ,×Wû¿ê~²Ó¿éù{ßýߝ¿ïÿJX=ÙªUNASNone?äê7oì"?LjL?ËÕüfµ?Ã¥õ‹¦€?À'€,šv?½wÆѳ~?ԅ0ÿs?Êÿ)!bñh?âJ³€v/?Êí:1Oq7?»•ŸÿòB?·¨ó?	Õ?ã}'þÄ%?´›!óMÚ?Ñ"*šnþP?²×3øÞ1?¿Ž "ÞD?£½Š"ÑÙË?ÆuIèä!Ý?°ÐádaE?åÏüíº:?»ñtfæÂ\?ÂJÂ`2ö?°ä‰uÐó^3FGL J0918.2-4859@pó¿3‡?҉O_
ׄÀ9.‡¶BFÌÀ:¥£Ho?å¿ÖQ¶@
ÀÍ^m»@†Î¿Á œ¿Ù Ö²÷¿æÒáìĎæ¿ç¶hK2¿èýI¯vz±UNASNone?°®5"[]?°¾±>\.?‰ísŒ?ÁŽ~(m¾Ã?éf1¬ù7{?Å.ÙrŽ?Ž–'s¤‹?¢'õ»†˜?´è¥øFU?³Úتܳ?ìè'7(¥
?·n&³ñ±?Ô¤³Ìø¾!?µ\¼¹CÕ?ųmRqª?¯_
Iò;ú?à@ß¾/…?·]ß3Sã?ÓxDÊs?»ˆ¬·ùw?µ­Ùöê±?£«2QŒG?ãü±š]p?¼Gń`3FGL J0919.4+6604@bvwFˆ{@C¬ü'œýÒÀ:§¢m}±ÝÀ<»%}¿ËDzfoÈ@Øi2ɀè@DÀ
¡©¿ÞºÎ}Q¿×:´Z¿Þï`qH±¿ê÷Ø'D,UNASNone?î\Žá¿?°‰WŠMb|?¥¼Ô½$?®qp@!bE?'IS/[Ë?"Ò>õU³j?ï7í"ɹ/?•…Ìcs?‹ÂsµþtÕ?Š¿4A,€?†BC—"?B?‰ùNr¥?ë¥órÎl?ª4·¯ÀTÏ?¶ÉMjܐ?¥öWÀìØÕ?¨-þù†Ä?–,ŸÅuŸ?ï%…wKö?Ž/º'ÐsÍ?'­Ã~Ô$ž?zã)¡oØÉ?'ø{'¬o?‡­"D1ê3FGL J0919.5-2200@ol¯öÓ0"@3áÞ¬É!À:qÀY÷ÃÀ;¾UË
¯ì¿Ô9Þpì¯Ê@ÿä8¼µ@"ÔÒXR¿ïûM˜†–?ïMÁ`KÞ꿬ŒáõÆ6¿ïÿÚeÌUNASNone?ì%:À)õm?èÑ£ò˜?¸J˜aqD?ÁgŠrð[?š.Gí;i?¨¬'à]֗?çM&î-þ?Ò2\9ðã?Ì/Û!?Т[W¿£?ªÒÁ5°Ë–?²›!-ux?è${*ê¶?µŽv=ߍ¨?Æ{ÿÑMd?´¨On¶ý?±ä''?ž8Óo+¶?ì3Gí"H˜?ÂÚ¸_ù?¸ˆšésð?°DÕ¢'š?—t™ýÑj?0.V«f3FGL J0921.6+2339@iœ´¢3œ@Ej˜þi'À9ØüvÀ;°jš¸¿ãðrô
Ë­@FŠ{ïd§?ÿ¢Z± I¿ÐÔò׿´¿áéÈ]ÒC.¿Ø¨b†¿ä<+{.œUNASNone?ïêõéÂ,å?isHšØÖ?JÇZXaû?Tԟni‹?\°Oeƒw?bÇKˆo^h?ï¾cæ©^#?|Ï­÷[¹Ò?oŽîÛØ5?qb4#9ê·?q•=Ă}?sŸ3+ùm?ïP~.H%?'ž@¼€\?t`Lw°?uÑÀPÌ{?Š‡À'öFà?yf)JÀzl?ïxo?ƒOå6GÁ?C¤²·n•'?Ccõ­p]ê?`8'b}‹?'ò›ßQô3FGL J0923.8-5154@q=ÈK¿òS;C£À8Íg<O;§À:ÊPrß?â ¸tu7@
GWŎ¿÷@`t	¿ã³íÅ벿ëuÖ?!¿äºáÊ#¾æ¿èÌPi`'UNASNone	?µªØW ?·Y(:К?¶n
á‹ñ?¸±¡ ۞?ê|ã8ÿKo?ÂüÜ~?e?¥ø‰fº5ö?´ZÚ³3§à?ÐÓz¸y¥(?ÊOþGÃ?æ6º
WŠ?Ìkp$Ù?×f#?¸ñßFøÐ?Áñ3bõŽA?¨M$Òk¯Ø?ß¡T6øD?¹ö'
6þ?ГúÓ{2Í?¶Þ!"Jb?»LVñòž?©­ Ym"S?äLwÖ(F?¹öû]Ê|§3FGL J0928.3-5255@q1MjO¿ötڂ—õUÀ:_UÐìíÀ;<ÔL?ßcOüÒ@¼HKôL?úgΠ·p¿Ð¶*
ðƒ‹¿ïÿ÷Dx2Ÿ?ïþñå,Œr¿½s54rÖëUNASNone?îkØ·Tî?±}ÊjÇJž?C
o° ?GR'Øݼ:?¨öLKYJ?±oQú3Ð?ÏfD®¥?ÒᏩª£3?—$Ò^S? µ–uZ?çmož€Ad?Ò×[mÛË<?ìT€=n«?¤Õän¶6ü?' ™¤aòÓ?ƒoÞ4wá7?¸³×«r&Ï?£zT{­;"?î¾Éj'Î#?­-ɅH^?ùýðÐ!?*åÓàê?¤j×féÓ?­.!Õ¬3FGL J0930.7+5133@d·—xW)³@F®$‰LD|À:ÊA{ËRyÀ<!¡t­¿ç'"'åw>@îÔ&2n½@‹ù€_
ý¿è‡>—Y<K¿Ô/¼«Âf¿ÝJ@(l¹D¿äÑäª0UNASNone?﵃çü?"'}H×?{£$‡ö?'{š§¿?cµ\´é?jõxüÿ?ïg‡ìv|?"öÿ»á?…í~f<¦®?ó;s'9È?€0ž¥º-?ƒ©1"p$?îðrŝ?…EÏÊÌ?"àÌm-?‹%8ߕI?'3}äAÑ?M|a[Ø?ïzÖ2ßxˆ?ƒßåŽöNx?i‰ïÛðOu?f'2Ä ?Šç÷Q%Ê?¬Ó箞z3FGL J0931.8+6739@b%M:'£@CâöÕ®À:ZxyŽaWÀ<:§›ºÜ?´>xt鈆@F[oèEN@T1ÿ¬s?¹hBý‰5Ò¿æ	8Ö`Il¿Þ¥LàÙI2¿á7vjP¼íUNASNone?ïÎä¶õò? Òó¢?góÄ9²=è? ¹‡¶p?jWWÐV?jÈQñf}Q?ï‹Û­3@Ð?ˆû?öŽô?|¿&kn?~±rIMNÅ?}SûP)F?€;†xák?î¼}õ?hs?'î)ÕÌi0?ßró"9?‡'ÙÀÖU0?—Îd"]Y?…HHððÂ~?ï+Rn­Š?"6‰¿«÷?qi6Ñ?oŸ"¼`™©?–;d¥^ªÿ?'Ëså.X3FGL J0935.1-1736@oOö©?)@8²~
ÇÚÀ:#×>?Ö°À;MPëªÞ?ؾ`Èíš"@bŽëjÈ?ûúp™?ïô¡›¬Õr¿åU›d䠿΅.jC<¿Ý
Wna\UNASNone?ïí¿±Ö´/?r̦æO?â?2à•ÜÁUd?6Ž{C¬ç_?_ÈvÛgM?r9$€xH?ï,@+ãÉ?¨|ùáuŒ?‡,æ.e
b?šL²Oĕ?ÃÆ¢b? ¸Í6‰,‡?îçTö5x?Š)𥣠?‡^'c?xSÍëΈÄ?—†±ðš'H?">Ñûç?ë—)gfd?°A	5ø*?…G7€úÀÊ?‰ýº²ç\?ÀNè*Rºa?¯•D£µV3FGL J0935.2+0903@lšmÚÏ@D.÷<ÉÀ9àyçLªÓÀ;ÈÓÄ7ÒÕ?õRl>A¯"@׎5bbv@8	cr–¿À.(Q­Ç¤¿å®Wa™U°¿ë™ISþQ¿ïÿÆç'
'UNASNone?íDö<bŸE?µ¡1Á0&?³'¡'úòZ?µ$ž~j?'­dO€œ?†L¢Ð¥U?äcý¸p[?Åþºh}H€?Óv.çPËd?Å؈-?®·ÙòŸ2?ªXÝ.=€«?äózIJÇ?µbû$Mæ?Ð"íB»ŽÆ?²b‡"úáä?·ØtÏ{Œá?£d·$;6?؇xZuú?¹©QÑà†®?áʒT÷‰?¼ªù6Âw¢?¯à©?§¨ǜÿß3FGL J0936.3-2114@o³ÿX:S¹@6n¾‰¬½À:`'b"sÀ;¹ö¥ä*·¿ð5§=h@ǽµ'®F?ý|@€M?Àømºm¥¿à
¶¡è´¿×¿Y±¿Ü¾¬3á?UNASNone?ïõùwß?V)ÿ.ñ?8^Ôò¯È?@çÏU5?Kì-<ȝã?PÞ¥‰E=?ïÅ´Ž	¦?ș‹Éž?d7LDëyb?gâ?¶°¾Â?s
Ùð?y1·÷ž?ï8"æÐ˃?…¼¥Qïæ?†.µ«x?}n¾ÄVî?‹È À§?yixÍóÝ?ï Lr¦-œ?{÷&éD¥î?t2î`Âì?!î`9J"]?‡±úð—צ?{Ѝ&z3FGL J0937.1-4544c@pô ě¥ã@^']Šõ'À9±aB:73À;A€t.¦¿Í.'¹5@dÆ(Bê@닠\¬S¿í°½wš@¿àMà
õ¯ù¿ßÛ[ž"Þ§¿ÞÛÎJv=UNASNone(?ﵧ¼F1O?g^N›t?_úz$¯Ãø?böE"Ã?}-ƒS»gŽ?~߬¸ø"|?íOŞ"èB?µÔÑ \µd?wðÑLŽ?jîì­#?´Å÷5
?´çÜ3®P?í¿˜W÷¬?›|¯ó<k_?"l¸ËIr3?"zÐl&•Î?©Ð"ÔÛÌ%?–n
ÀŒì@?îŽË©ÜY2?"B»ïX?O¥o:ÔqÇ?Obc±Òς?¦"¯¥O?"é†~ñB3FGL J0937.8-6407@qºwÄ\»ÃÀ!"Ê`"À9Ó9¾hÀ;…jŸ±
Ï?Ȑ}l£}"@m¼}cÃ@\Bjy¿âRD###¿ëI"×ã¬7¿ã]W</ŽÂ¿Ú^žRÞ@µUNASNone?ì~Àóp°×?¹%é3T@æ?X¬ÐñÌÍ?WÓR$ær?»§H6²?¹''åÜ?ëÔÉÀ´?Á%ÃRŸ?'d8¶>?šz‡%P)+?½3"pM]?½öɓúòt?ìû+ º?¡Zâ–ù¢%?—³)8Å=?'"Spœ]?²b)ر ß?iKÓÖ¯Ñ?í¡¨ åmJ? 
J^é
X?kdñ-?oÏ*ý«"$?²ò`yn%?Ÿ‡ÜË"­3FGL J0937.9-1435@o8ÅCk@;48L`À:Kç]qËÀ;¹¤½º
R?ãC^ÿƒ@j3PåJÈ?þ<¶úS?ïý:"£§¿Ù"´¥Â%¿ÚÁlÇS'"¿è°Iۅ9UNASNone?ïÎR¨(û?|[•ï˜Ç?ruÌÀ^Ä?xυuϋþ?Y†<{YÁ?a~çGlß?îW׀_œ?¤:՘ i{?œ %@0Ï?šý?äjN?'Ôß÷³ÛÁ?–4åƒÀLl?îxS"®R²?™OÂú?›#Ï¢É-?'È•çð`?•Ñýڒà…?‰›µ?ˇ?ë¯ñÖKR›?¯§&™.Ɉ?«…^‡B€B?¡BŽ'öoZ?´½Â
+?§öqøÌèµ3FGL J0940.6-7609@rCóÿ¬*À1lÙÆ°SÀ9?ÎÞ¨À;tOÞd¤Å?½)7ÿD7@ÚÂ-âf@H_•;ç¿æðýlŽõ¿ÞG¿myç¿é›ã±¿ïÿۄ—÷%UNASNone?è2 ށ;?ț2¸y·?Ìáï⊘Ï?ÇÓoûìo?'œ}Û?™³:‡PP?âÒÉ£ïú?ΉüßE[?ÐH.i"H?È0Ò`Ñ+?Ä'Kž‰?½ò1@?å1:Z•ÐÚ?µOý4_Ï©?Îh»lÊJ¢?³,=€‡ŸL?¹¤¶Q¼ãî? Ž>Î¿?á[ßꟘ?Á¥ßV¢ú®?ОR†D?ÃË%õ´Þ?ʃC°w5‡?µÀD-¬3FGL J0941.0+6151@bïu£KÜ@EŸÝ]=ȸÀ:€º¥'ÜÀ<
±qýs^?Ú9üSUÆ@¾{
L¯@_"ŸèN¿êô
$ù)¿âe U,y¨¿Ö¹âÏÃw9¿è–ËFm€?UNASNone?ï×îE‹Ðt?|rK¿2º9?k@,<Å0}?y/ñ‹Sú?Y£nÔ·–?aó|Õ¦Ü?ïÕÉ8³?–×Aà6¾·?'fòd¦?T?'•®ndu?†¼¨è¯"?†_Ѿ'×?ïš	\s?Ž¨©ÖÖÞ?‰ä¨ÁmÜò?'çKÆ«'k?'í8^ƒ??ƒ‰W8‰´?îÿiùþ£?"DdîN	õ?†""PŽ(F?8£¹GàÎ?"É/§y?xŒ·¶F3FGL J0946.2+5209@d7Ÿ©~@GÁÊB®Ñ9À:/þ|rAfÀ<ãðÖ?ä²]Lƒ³¡@ЩIëñ@á'uƬ¿ç/ϓ ¿ç:`ϒi¿ïðŽºå»þ¿ïó¨d@OUNASNone?ïÙ©^!g°?ŠmèÞüE›?oø÷jwq?‰ÉŽCr#?Iv©Òef?X
JI°(?ê_÷=ýHD?ÀAŽDô!?ÁÕ̎…«×?½M…Œ›ùD?¢©YæÌu?¡ØF?Ä¢l?îPÁ–"gÍ?•DŸ}Z¿?œyXNÜ?Œ‹[Zvd"?™ÊSãd†š?‰‡§§ÏP6?â*Í_sÀì?Âïÿî§ó?Øý4R+?ÓΔøË»?¥j8f3Wá?¤ (!$3FGL J0948.1-3641@p¬/ƒ{J#@)üõ:uGÀ9N]-؀À;"^‡tÔ?얦/ݛÛ@gĹWúé@Æï¿kn¿ç¥ASÈ¿ê÷˜lÀ?¿åJªn÷¿ïÿ²,(UNASNone?î¹-"‰?£¶þ¾ö	‰?—Ò^ÀÜw?—1S|Ë?'Öê{Œ²N?—OErØb?ؗ&3) Ö?ÈÐ1ÁU'Î?Û8Ÿ^3'?ō´×-­_?ÈÍBZñWP?Âú<ëç˜j?ê2~<F\á?¬<8^é~Ó?º!ÑÏX†í?£+jÏ´ïà?´J<Nt'?"	@þÕ×?ÚÃýî'¬w?¸w"Ø®¶?ØÅÄ –ŠÉ?»A|À°Ä?Èì{⃑ƒ?²Îý·ûÄ3FGL J0948.8-4243@píƒ<`Ÿ@ û¼ÓZ…ˆÀ9ª¨ëF4˜À;u­Ñ_Å¿Úç'euz«@
;R'rY@ñ…@œ'h¿êeÜVòD¿ã9¾dv™‡¿ß0…_a¼¿ê(,"dËUNASNone?è$ûãÿZ?Æ(Ûbm±ª?±ñÕ&4
y?°­Õb×î?Æs%à™ûÚ?Âþ7
!?"?ê˱êÅÎË?Âóì$˜º?"B
¶%Æ?–%µ7|3—?ÂHöž$Ý?ÁÝ}¼Ëƒ%?êàËh¯ …?«H"VR7ë?¯sêçÁÍo?›•Hvï]l?¹?¯F¦?£²o»/?ì£]Êû?£G߃å@Å?ƒ 4VTq?{k2¯Y¡Û?¸$u£?¢Ðæµ¾e3FGL J0950.4+7550@`í(Œç°@BD–Ý&·$À:Ö`"•À<=%ÑJàÏ¿ì1Éc‹À"@
óp˜nv@'Í@¿èòW‡´¿ã¡ãÙ?8¿Û™;‡·ç/¿ã¬¬
VèfUNASNone?ïª)7¶pO?¡œÖ'•]?x{…áYe\?‹'†@-x?roÞCns!?Ÿö?"q?ï¯Ó²‡˜ê?'‡l
ø?q'|c] œ?r˜Å{§©}?v"ªXÖiö?z[næÌkÛ?íþŒ%h¢?¢ݯ,ä?¥ÉÖ¾Saˆ?¡Ló&"†?"šÍÖDü?'áÂö`
G?ïËR®,&h?sHê.™^c?7+AãŠ?9A}ÃtÜS?xå§8­€?rµÒy=º3FGL J0952.8+0711@l·`—Ì@E¢}sÉÀ:sÐIYÀ;µ™9øI?Ô£xM¢'æ@
jT»ï?û0©ôg?ïùcñÁùµ¿ ['îËi¿×®k@sk¿Û~ˆ&ÌëUNASNone?ïì'uðž?rsNË_í?MØ)(ªªð?Q	ž‡=±?WðÿŠn‹š?pÁâ˜Ë?ïyÿ¢¾þ/?œiÈ9ÿàµ?ƒ‹¾ª?™¹Zȗ£?{豝,Æ4?€•+×$Ö?îò¸èð?Š†w±î4"?Ž'fÉÐ1?@›;kV\?'¨¼Ì}ùØ?€µ"Ù?î¤×܁?¡S_ïèq?'úôâÿ±?+aŽµª?¦h8Ô8?3U¯¥	Ì3FGL J1002.0-2837@pyæ{_ï@5¸Ç\J"À:*ˆ«€À;µØÿàöO?çÇ(¾Žñ@GP×3@œ	ßý¬?ÇVùÌ_>ª¿è`ë'UÚR¿é!ÉÔIï¿ïÿB¸·AUNASNone?ïtm&#ÿ?••ÇRgH?‹-Ùs¸ú`?"KD'ä\?nÛt
Â?x‰"æ,Rl?Ú&ӑӱ?ËÐ=kYO*?à-ÌB,–?Êu­Og??µöO¨Öç?´A&L"¡?ê©>/?©3™5™ì?¶ò[B'€?¡Ê>Ïiü?³Ã³AßöP?Ÿk6SŒ,?Ñ#û_é?¹8J£ê?ã2;Íô—?ÀOØЍO(?Àï¹mÏý?²;ö¹év3FGL J1003.7-5215@qlKƧïž@–ÎãþAºÀ9Æ)É'%ßÀ;7]ig¢§?íb¹æ±6@˦‡Ù@{>ŸÍæ'¿"±h~Èô¿Üþ?FοåµjlÒ³Ž¿ì•h.èuËUNASNone?Ç6q§wu<?ÀsÇQZèü?é(DrsÀ*?Âmç‰
ç? ¡ò:æ(s?¤¶,Pe?â؞& ™?Î0†·X¬?¹&C@—d%?·hÚׄ‡?Ô21åÅ?ÊîXݸ??â&d‹ìÕ?´˜ž{<!<?ÓA3¡@Þ?±ö2´¤a|?Áhÿ+P"ï?¥FÄ|¡AB?â¤	DßY?µl5·LEs?ÈÇ`rË?¯ÔZ½1•J?̨Ï:znÒ?®ýîbøÇ3FGL J1008.6-5706@q£*\|Ù¿î3†_€>À8&Ô©À:(ÇÅüÎó?ÛbÕh¸âE@
Ÿµâûba@ˆ€—•¿äúEoº'Ñ¿æy™¨s¥¿ëAÀáÿ¿áŒs%¡UNASNone?ŽÏrÍIK?"\ÿ>7?Ç^m ‹²£?Èâ2"¿>?é­&̨¶1?Ék0ÌIÌ÷?°Ï3ÜãÈå?¹ |Tcà¾?Ãõß_¦Hü?ŤòٌÞø?è衬yô¥?Évö>?¾òá‹9Ž%?¦×¦üE¶æ?Ódnëv–?½QOOÅí?â–ñ—#ñ?¼ê<l2¥7?ÅÚ¦=" ^?¹DE-—‡$?§Ôþ"œþ?¥3hö6õ?é‡…þ?¼@l™ü,63FGL J1010.8-7645c@r`ï~=ÁÀ0¼øµˆãiÀ:¾7ޓŸÀ;o	µ‹g¨À7º¬cˬ@õ&Ûa:@sð?m©&¿ç–î÷ø}¿ê¬kÉ°@X¿åÖÆ]xÐ?¨ž€Íߋ/UNASNone ?îO¦qmÐ?´é'ᒕ|?\Îø½B'?f—©]5²?ª(ahHò?´¹DÌßy?ïÆSfšî?~(ƒÊxs?Qá·­~¥H?Y3oÑwiÌ?x^aRà;?zçaCo?ío¿o£_é?œ)dü‹C?•EÃíkض?ƒAû¢AM?®a'?˜Lñð§Å?ïµßG;¹?L·W"c>ÅÊW¿ÞV>àVü§*?'†ÑzµŸ?Lnkyo¾3FGL J1013.4-4008@qRÇ%Ä@*µÿÅGÀ:=©µpµÀ;ª\™'6¿àvÃá@3%>Röó@Æ ‹:Ü¿ãM-M:¿èw/òêv_¿Úzƒ9L¿Üщêc®UNASNone?ï: (*Ð?§N'|('Ð?WGàÓX?Œ™{SïÁ?—K†|˜Í?¦´f[+î?îôZîDf?¦÷Ç:¤
1?rê*…¦?z콋Úʁ?œì§¬Û°1?¤Ø€^›?î7KqΕ?˜7Ÿvõj?‹«p`¥?|óag}U?¥ ˆÆþ"×?"¡§ŠyFÐ?ï.˜D©›?‡Ô2"¦«–?8Áô¢Ý0­?=­èþ6U²?™Éï¬ÿWÞ?‡¦9F#3FGL J1016.6-4244@q/È÷Q@'%WšñˆnÀ:#ÜHjÒÝÀ;'Uœê†ò?á;Ó*½@x|¦CÌ?üƒÒÀVǸ?ï±jØÞJp¿ãæh4æe¿Æáâ	í6¿Ú0âÿ$tUNASNone?ïïAúŽ/¯?e±}¤÷?*Ï)¯Ï?+Ïu×V›?^"%ÀJ½Î?dÞÏ÷ J?îiÛMœùq?²bpë.?zX!Š§?'úi×^O4?¦I#ì7œ?±;Y?îáïʗ‡^?ú¸þa˜|?"÷)Ã'?yÒ¯Cñ§J?™FqˆÊÛ?7ÿ[ËK2?îHf@1? 9ÝÁSXp?a5D?i͘¢õ·Ã?ªn!«÷»?ŸÛ£éõÒN3FGL J1016.9-2653@p"æ1ø @8sÀµgUÀ:ùã†MÀ;ÁSL®.|?äøã#%t@F,6ê¢Ì@×(Ÿ[zz¿äšèù=f¿æ
Hy&Ä¿ê²!óR¿ïÿå|WO®UNASNone?ï`üÅVõþ?¨Å/cª?wѤùo?;*WkzÒ?‹×üHeÉ.?§OPâÜ"?çòh@®#ø?À†×m€X«?É&ÁÂq?»Íø
kH?¬>tìãü?«(ìÿçün?줇¬ÏW?¤u¡tiÐÆ?¥´­ÁË[?'ªÆÁd:?°k¸Ÿ–?  m—¬¸?á®qƒYj?·ÅGÊ.?×Ps%Òȶ?¹¡
¿Ö'?º¿ÜšÜ?§IØÜ<Sj3FGL J1018.2-6254@qç"ßÎ1QÀ'C¦GýÆÀ9–©$Q!À;A#·;k?='9@)ÿæ)À@Š½¿¾œ]¿çXQ¹—L¿ì¯ \†ä¿Üi"Ei8¿èø²JYYQUNASNone?åÓ‡dî?ÇÆ#y'è?¹Æ¶» h?¹Ö€ 8Yu?ËÐH8;?ÄӄÔâ9?Ƭì?ǁ)½¨ÊB?ÐÕ\ßåp?Âw¨Ã†‹?⦏ˆ-?È:<Z"(?èqéà=+Ÿ?¬Õ¼/š?´ý,æüÿº?Ÿ¦Á!is.?ùŒѩ?¥¾"ƝAæ?ÚI/··§?½ÑB­>Ï?'_>¬fË?»´Œ¶`ú?Ün ¨ò±ô?½Ì]Šïd¸3FGL J1021.9-5815c@qÄó#x«
¿ìùcÞ÷œ¯À8‡7ø"Ñ´À9øîº]^€?ò¬g|õ@
pò\ÔA`@iŸè=A¿ê¨ßp¤"¿èPÒüøʾ¿æ?˜°ªF)¿åX£7ÜUNASNone1?},7CðÚ?€E¼sâ ?Ì]·"8\·?Êi€!Þ÷b?è®SÂÃ`ñ?ʝúhÀ0ß?°Y@‡›?¼ úéDˆ?ËãÎGwÔ?ʐàÆ`_?æûäwý.¨?Íi¿›'Šƒ?½¡êVRé?¤â(©>?҇ÑõuDN?µýñ"ª?ãÙº{;?¶"Ò»©Wû?·¦yøÎi?¶'ÜãØ"?¬$K"†M´?¨û2ìÓÆß?ëHì£áX?¼5"½3k3FGL J1024.3-5757@qƌ½D¦¿Þ)VÍÀ9š‹1!
À:.Ü:(ú¿Ñ>ø­jÈ@ò¿[Ëñ?þSé Àiè¿î;[¶4/¿åW#P?Å7ÿÒø0¿â¾ôUNASNone?¯)ÑF"½?Áúðw~	O?ŒÐOá?"À«w5|?êãÍ8m"e?Âý,ðÄ®?ÀzÛù•Ñ?ʚŸåœ
?¡6S\Ü?©7`¹r_Í?êÏè~5i½?˛h™YÇþ?ÑÁ†w•I?±e
äŒq?»¡ÿ®ÖR?§.ªÌŸk?ãªüδڑ?³0:~1?ÜïðÕ»H?ÐæÄ,VôÚ?B†MèÍ}?RK=!Äÿ'?áƒóŽö©?ÐéFË®-j3FGL J1024.4-4545@q]¼ÓZ…ˆ@#®šõº+àÀ:dú:þÀ;­â1¸ß°¿Ù	­Ä°ú@
CËPuä?ÿmVàa!¿änkͥݿèëÀJˆdh¿×ÄöCÏÊ¿s)â4d¢UNASNone?îðiU-Þr?±X$&Ù°?5|è# ‡?7ÚMCqS? ÎpÜÛØÅ?±U¸xª' ?îFûû;y?²3¾Lõ/c?rÞ¤Ôâq?;7î6?©Mdn‰|3?±µ•'¿?îCÛn?šD8+PÏ?"t÷˜ƒì/?s©ÒGôô@?¦±b(#
?˜8Òk*ÕY?ïŽüjHÀ1?ÞÈ8[ó?É$ʓ?)Ô¼'ß(Á?ŒS$:͖?Õq<í¢ß3FGL J1025.1-6507@r#9ÀëîÀðÞ	52èÀ9g½ò>v]À;OÅ?é$?ð1©J¼'Á@¿r/r^l@Y© ¢ÍJ¿ä48/¶é¿ç
Šån%Å¿ïõ2\¸"?ï!¦mèfUNASNone?íÜöÿt/?·-VÂ?ªEý'Â"?°ÀW(`?£ì2þF›?¨˜6=€±?é>ú^?Ðr/ð©%õ?—
\{€¶?¦h[ê§Ì?È$Ó¥ˆ&s?Íëý¢u¹?ës1W·wZ?¦uýí[q?®6ˆÆ¹Õ?™.‹h†?µK.}àèD?Ï¢:ŒÎ`?îïû04ä?¥¢0cbÛ5?i¹¿µ()w?‡é½¸
ï#?žÉb¾z°?¤ybQ‡3FGL J1025.7-5659c@qÁ;÷'?ÜÓ¢©ã"À9·
èaÀ:O|N/7ü?è
j®–ù#@U¶öv¿O@'Ÿûž¿ã]+Í}¿ë@%§ô¿êöü²e¿äZW'=°UNASNone0?"wì|溄?"í{÷Òº?˜.~Hãóì?¤qc¥œû?îì¬[ÅEv?©›®-.—? ôš9¤?°º4'}|ñ?­Y#Ô˲Z?±¶nR/?í*.y¨°?º9uE4?ğúf	v"?¬Cóν}?Ç=NŒTÓ?²Rî X?å2ڍD?·-€óqÒÐ?ÏSx™&N?ÂA†‰õR?¢£Ýã? ^\9ºù~?çmQ(Eÿ?»-ms	3FGL J1025.9-5930@q֍"M;¿úûh÷:^¡À9õ@‰]À:vc ¹HŒ¿ù\·%Eµ@`?
1@¼¿Àéz¿Û3_Œò0"¿åT]/¹‰­¿í\ºPüпÏeo+ÃUNASNone?½Y:¦~¯?¿°ˆìfà?´þ»Û?·¬í Ù?éĘӴÉ[?Åv˜wÿï?äÜ(æ~Õ¬?ÖCW˜mbã?"ŸÒ¬{?©‡žœøà†?Õ"5׌ø?ՑT+s@?Ñ·ÑvÏÉ?´~ïZé*€?ÄZQ‡Gü?«š7ÿ¨?â_ÑâÆ?·1éZBƑ?é1éüHÊ|?–³–&'$?4Ði'Æí?F–M²gëx?Ë.&¨­?•Õó)F3FGL J1027.8+8253@_øA [À@@e¡"úÖËÀ:y¤O\_À<çCp˜?Ó»v«Ô/@
ܲ6žw¥@•¦_Р¿ã¼Ê}+¿Ùw£—–¬w¿å臿Û<÷"œô(UNASNone?îÅÇ&LÝ?³ø^ò'?pÁ=3»?³³Jê?E?ƒ­êNT+?†þ[<]ì?ï\ç)vÃ?"z(渰M?…}ÆIîë%?ˆ™eCŠ'?ƒHoU³dC?†\í"k¿?{›]…?–¢ŸÁûè–?•dE~BzX?"¥NG¾R?˜JëQÔò?‡oECì0?îìÃ~ƒø	?"2)€¦ßx?‹õSêC¥?ˆIù±s?"læ:_,J?Žz'¨4QU3FGL J1028.3-7419@rXú$‰LDÀ,=Žc|À9ê)€,À;X¸þ¹¯¿Ê›IÁƒÝ4@OFǏ¡@…:Ÿc2)¿ä¬Ú¼N¥U¿éÝ\0F]¡¿âHS‡Ö<|¿ïù۞ÕKTUNASNone?îˆü¿–'?­¿RK[Þ?sa¬:ˆ??x­mlæ?«Å£þL…?¬ú€4Í?êFzçàZá?Ã+
ê>¿?³é6ŠØ8"?´$y*€ƒ…?¹âò6$ðq?¹c—/W[A?ë¥sçDw9?¤Ý9ºNœ ?ª‹G~!È}?'(/6¦ò?µŽ½Ëaô? ,>:*ñ?æçbÄùÜ?³Û!ÌÃðJ?¬ÿÕÄ
M?£-pN"?Í"¦(½>?²>eàN¨¤3FGL J1030.0-5809@q҂ýuâ¿Ï¶™šróÀ9žü¯égÀ:H?³t63¿å­¯è)cj@Q>kµ±?ü­9~ÑÂ*?ã}M\¢¿æ_µj¿ç«®TÅ1ֿјšbŽ·áUNASNone?•.±·1Ë?¢7Ì-À4?t뉝3¦?€KÜDɳ?ï,³`GàA?¤.Ò‡"Û?Å÷ˆ€û1?ͱ¾€{ï?".;ô!ž?›\˜ÿW•7?éèô (?ÍˈÅJ¾á?Ë֞B¸˜ç?°ªW,umB?¹åx0Oý5?¤8V,{Ì?åÍ©iGÚ?³—H?îf?ãÕ睒Ð,?Ǧ½"Aßû?BƒýKÃiº?J–ïjPÏ9?ØJîÆ4}ô?Ç£ô'Îph3FGL J1031.4-5855@qÛXâe,¿éôّmäÀ9/Q˜y*À:^2»>/?â,ù|rE@
­o‡l@®<_Å½?íc·yBP¿ÖËïΣ'¿ãPÊs^Ïø¿ÚY°~7UNASNone?É¡®§-¹?Ãò¥"#×:?©]Rõë8w?ª-Ðû´éö?è¿&ÕÞ1?Ʀ­xp57?ÁesØۑ?Éëo¶) ?¯ÄqÚô?µc‡0T?éÃ…i©Ú?Ëáö(¿†?Öd@"§‰‰?µ­.¬Ôí?»Ì(¦Íf?¦ ;UØþ—?á]æ0—a?·5BÝ»ãG?Ù@Ze!œ?ÂúDZy?¤.aTܑ?¡Þ¢}^ĸ?â
¸!h?ÂA¥1ÝF>3FGL J1033.0-5945@qäîcŠ	¿öÃdٞlgÀ85׈±ÙÀ:k qäI?ᬜg`@
*l!à@	ohی¿Á žXùžð¿çe2´³%‡¿èK4ì=Lß¿ê­ò$'ÛUNASNone?Ÿªçfgd?¢MŠ-Óf?Ú
z%EŠ?ÏÄ£?~^2?áýi¸â?Ïï¦ÐèMÃ?žïׇæ°?¢êNË­ì?Öuí*ׯÎ?Ê0U¦´›{?ä@ë×èã?'¦…Nâm?ÂoûÎìe[?©'Ìúî¶á?Ñ?Ê[)Z?±dE™Lk‡?âÄÞ°[ü?´ò"o¡+?´R•£Yî?§.Øq?Ȭþ6œ?¸¾üÑ#rÈ?çJ…Ëí;?¼Ü¿xYri3FGL J1033.4-5035@q›—Oß;@	U./¾4À9TãqT2À;_	ðCÊZ¿×QÏO!êû@¹ÿ´€¥­@'À
¼Ç¿ç³ÜæËQ¿ÕP¾Î M¿ÚLfó •ï¿á¸äÒAUNASNone?ïWÝÌá-.?"CÇ%iì?d1';&۞?aRf™ÂgM?'~u~Ñ?'RoØâÈ?íaû2ñ'?µ—êmx?}X.ÂD'?~SûÆ?µ÷m:D*d?´æÙ">6ø?íõgêÀ?›0"ÁÅ\?'íp'5œþ?'ß"3…Ã?§2Õè90o?–adK±Ä?îD¤êd¶?"‡²Ö"_?aG 'OJ?_qªhÌp+?ªŸc©4Ä+?"B' ò¹3FGL J1034.0-5731c@qÔ·éùr?âQ+6¯ÆÀ8‰Sԓj«À:m;Ì^èÄ?ñ7œvë¼@3Qƒ«E¾@D¨ƒñ?ïþoïÒ
y¿êBpI³—¿åMÞzýªÄ¿è´MŒÐ³aUNASNone0?ÄéeŸ«¦"?Åí5 j?ŝë¢ß?Äws^J­?å€T-Á?ÍÊ-h}Î?•Âêãß?¯'Û	²iH?µÞ'X'µ?º"[Ø2?ì›O÷˜Š?À3"QЉ?ÈÌïrºPÍ?²à8ðs?ŀ…¥ÉÐr?«Á;¿áÂÑ?äl¢¹Þ÷°?µ§vøNË?Ãuaÿ‡·?²H²áî?½ ~;Íß?°ì¬vÜ[Æ?çn­dX¤V?¹Ës:³3FGL J1036.4-4348@qjÚãæÄÆ@)9+6½+À:(ÇàÔÁŽÀ;²Y¥Ã£?Éx§À'›'@
‹+ÅUµ@6èßÒãè¿êbägYfµ¿Üõ>.þ‰ø¿Ñ2VG¿ïÿß¡ï1.UNASNone?èûqo)J?Ë£i~jµ?ÃUÓúD¾ð?ŹƒÞ° ?±wÔý7Ì?¹Q4'k?çe×٘?Éô³äg?Á(÷™úrˆ?½í )1å}?Âaq	ª'?Á_›&QÁ+?èWË7¬V?´î	õ;»=?ÄÛiá›H?³­ö'ð›â?³‹jêf¾?+ŸüÎ?ë]°Îƒk#?±ûø?©Ìmƒ›H?¨lAâÛ?¸,C"ÙL?§}{ÿÎs=3FGL J1038.0-2425@p¿á2µ_@=;qdÇ)öÀ:29Úí!À;ÇÏ'ðßÒ¿ôtÞt"ý@PÓw`ߔ@,\@Gù¿çO•ßR¿ãlnÌ&J¿èøʕÿŸø¿ØFc]˞UNASNone?ïë.üäUö?gxÿ±6v?[é7ÖÄû?cËp7?Kqßþú¡$?Rá7r†U?ïÍg3'¦?zX!Â*Çj?cÒϛ©¢î?gÛ]¸_7ì?nÅüáÅ·b?sÅÂ(|€ž?ïNþb½7_?ƒ	#+¡
?ÀE·ßÆL?wHõOðõ ?Š€!˜ÒaÏ?xnƒÒéÜ?ïÒÊhŸ?p"o‰d7?vÂúŠ›7?#0õ¦'¿?v9$íá†!?p||ó?Š3FGL J1039.5+7324@`׆`ÔV@DG(àÉÙÓÀ:fK†ýÀ;éäwä=,¿÷æ©IåÒ,@ˆŸã	Ð
@À6 %#ü¿æ6…sO‹Œ¿ØŸ¹ÌÈx³¿á¤ºiÈƃ¿ãÍ
ñŸÿUNASNone?ïëb!°´?¡ôÄ+À¦w?1x€AîVÜ?:·+›†°?bAÖ€L?¡õ?[€…?ïÉÈâ"¼?'!ìˆ9D©?gDPYwg?q,±Øµµ?nó§!Ìä?yÞàé~M?ïˆÿµ$•7?K¢'•?zîëó#D?v¶[דû ?€I@á ƒ?rt»ê¸3?ïä'ãŒ_Ë?fˆ3û¡?j}ù¿ð¶?ã²'˜?jÙȃÒ65?f4x¡)û3FGL J1040.5-5926c@qï™Ã‹«¿å¼^pÐÀ8À,ºs-õÀ:KŒÚw?ì/±>âúó@}Fößoè@U— E/_?ïÿÒ¯Kè¿çœ>˜ÍÔ¿è·ÚÙ8C¿édz"o!UNASNone5?º"]zr~|?°žÿ÷N?ÐíhTÐz¦?Ð2—†LSÇ?ä6à&IrÝ?ѕ62êvç?€wД>a#?šñâ®3d®?Êêš´òÅ?Æëòµ…Zÿ?éz6ÁÉË?Njð]Õ?À@ÛßÍW?¤¤[—nÇ?Ë˾´Ùê?°¨ñÒ´	Õ?äýÑÊp?³:V3vÊ(?¨2í%/Øî?¡¸'"¡"ö?Ê/.òÒq?½§×þ–o?çúaðMÕ?ÀëkE'd3FGL J1043.6-5930@qõ¢£Y6¿áʇ㎰2À8'oJ:¶µÀ:ɵÁ?ï¬çÁ½¡@˜ü§…ëg@†ü L{¯?ïïð`OËð?Ø{W­C£!¿â¯G›¿àõ°Ý)UNASNone?'Ýø
˜e^?"cHS‰5Œ?§ök‰P%!?¯PÉ?í驆þ:ƒ?²W¿®Ëí??¨—Tióq?¾:bVé{?Ð#j¥†®?ÍÏ®÷ñûm?ædÙH.s?иuù'V?ÂÍ´! ?§éÓ?¶z¤ÖÓ? z!Wä"?è¬x;P\¼?®%¨"Î?·dbt	{?³ÿ)ö³2?Õ#­qR?ÆÛvçA+à?⌅ø÷(?Ƀ–ÙG}3FGL J1043.8-5851@qñDЩ*?Ÿ2±zƒKFÀ9qÁ
|À:¶,A§j=¿ãx×Ko®Ó@öôØ·›?þÒ_‡$!¿æÔ)9¬–n?ìS¤øûÝd¿éúvÚ¡X¿Þq'>|UNASNone?ÖGÚ"ÑÏå?Í®û3Ÿ¡.?²ð¾Š?Õ?µ½î|ãJW?â}ûO5ô?Ϟ[A(ý7?ÚÇïƒA?ØI_¬6y?ªkñŠ'Q?·Û1*éê€?àõ¸v¥Ç:?בŽÐ]$?à°W½}±?¹
hµÓ ?½‹)ÿ‹(y?§rG…Û"?×<†!Ó¹?·I®+€?èαf&Ù?Â×]?¯ì 'zø{?µ2,ûp¡#?ÄÊ]…ÝÊ?ÀÀ¨Ìh"3FGL J1045.3-6414@rIº^5À–§}‡ëÀ99ÀgmÍÀ;ú¶êã8?ôœÙ!™Ø¯@Ép륀@êvà1-Ÿ?î…а噿è5q—Ù[¿é°9é'BÜ¿í ¯"VU;UNASNone?À7UõùGé?¾|KFèÜz?áQ²–a:~?ÎS"ë¹?Õ@ïØ@ç?Í»ˆ¹¿)¸?±Ý£ÔMô?¼á\«Ïù/?Ý˲%Oƒ¦?˩اß?ݽñ»hÝ?Êbæ]=Kî?җD-Ÿkh?²#?£&Âó?Úè…¯ÖŸ?³ád:p"?Ҁ6°½ø?²5 Ò&TX?¾÷K ò¦?¬Ÿa:">÷?âïw߶?ÃQ
Ùtý?Ô=½xWK?Àóh!
'Ç3FGL J1045.5-2335@pуùd@>à¼8*ùÀ:gK-û»ÎÀ;Æ¥®zÒ.¿ÑOƒ@r@
ö"»Á¸@ð¹@}ôx¿á»`…É$™¿ä½'J®¶¿çÈóœDnÅ¿åäS'¢FUNASNone?îüè¼(?é?W©<#?mÊÁ)áå?~,()ºü?˜‡uÊ­ŠQ?™ûm¾!qÛ?ï‰+æ^î?Œ/ë‹Þ?|ö"¤6Ó?€6geîIJ?~sý<äÅ¥?®_¡OЮ?í˵½y²R?™Ø^ØìM?˜+B½
ã'?‰]y4¬Äù?§/Éßi	?'¼öß6@?îËM: ?" 3àƒ©?¢ÉÝL~ü?v…ÖÿI?¢þÆ'?'Ä&Ru3FGL J1047.8-3737@qW8›R~@3Á;ŸÀ:#`m(!‡À;­ÓÞ9Û¿ÖܙAÃ;@¸
n˜å?þR}`}ï?»ÀÝf‰2¿Úœ91$T¿Ë¬šlu¿çi øÈÿ
UNASNone?ïǛ1O
¾?—°4ãõ?_­!"KÛ?},#[æ)Ú?tG÷gÙ?Ê
xw³ð?ï|(ÝCü˜?"?Aââ´°?t=óÊj?s»wTng7?†ÖÏ!›¤ï?øØÙ¼Ú?îݲ:/qˆ?'>¶'†êœ?¦góëÓ¬?"ìÃúÓ\¶?"v"Àå#?…ÙA9'i<?îö?H	mA?'Š¾Òø­?\K'Ççb?Zª­¦sËÖ?Ÿs]âSáº?')UC‡Ïf3FGL J1048.8-5006@qºQc4'¿@ <½ý&À9ýýQÏÖmÀ;pŽÉ[ÿ¿ÖyÐä½@
@¶
Í@cƒ 3Ï¿ëhÝûÚh¿Ó4IèE=¿ã2>^4"°¿êÏYVTíºUNASNone?ç2—Ù³©¢?ÆC'êÆVó?ÇÁ~ìDæÃ?ÁBúﰆ?¶èCYØåw?¶`(DîÍ?ëFjPß¿F?ÀþüNÅ&e?•Ö'lê‡?—ùcú–\±?À4[ê3e™?¿"÷óFz«?é­))Û?­"0'¡æc?»´µë(âv?¤²b9îµµ?¶âËàA?¡p	?¼@?ìc¤2R
?¤Ïøk'Ù{?• å‡cä?Ši$­Ü4?·Ÿ4%–®?£e· ´»3FGL J1049.7+1548@luâlv@MÎ#žj¹²À:Ë*5]°À;Ò·£oÜ1?¹'ÄD©Wq@DÄyl'›@9Qx Ñ¿ÇD£¼ãýV2ø¶ò¿Ùô"U~{u¿íCWŒšUNASNone?ï,ý4DË!?›ˆòæa«?•!žaîI²?˜^»"¥SC?túìUáH¨?z&D0ýØ?ï7™¦O-?"­bLš?¬3éc\?‹u€ˆúpn?"±-b'Ñp?"?I;R?ë‰Ó¬rÿø?¨¤Ýjö1?¸'¾*~É,?¤šwá›g·?¦=HãÒn9?–³\֙?îrâ†h%Ú?™_0§/?Cá_Š?ˆ ©n9!? Æ5¨ûòž?"
T~Bá3FGL J1050.4+0435@n±
gb@J´Ø]ú‡À8ê'"ÂÀÀ;s˜~§?ð%²úh¼W@ªð†y@ÂÆ ‹:Ü¿äæ}MŜ¿åmÏ557¿é¾Š¥ñþ¿èéM¯VUNASNone?ïöÖçj`Ñ?KÀ/g5gÜ?G¬¿Ÿƒ¶š?DaýÖ±0?9ïEmò
?9u;1S6?ïÑÝ׀.~?{<ß]kø?fžï¬Ên?rhþï>ãj?gƒ8Ó›?n'ù;ñ?ï4Ús ¢©?ˆŒqÄ´@?…Hʊù¢ž?}fSd̜A?€˜ŒÝ²÷?€˜ÏqÀi‰?ïä£'@]?q'¬4(´3??suX$úº?N{ó™1A?gnjžJþ?pX,¹+Ç~3FGL J1050.6-6112@r {5*"¿ú¹ýl§ÉÀ9gâTÀ:"Ö)làÔ?ñ^¦ß'mW@
á>µ[E@Ñ.à=B?ïþò7Y¿ëç…* åÔ¿ïÿí›ði?ïþ¾M¥UNASNone?Ր1¿+|?ÕO >ϕ?ÍXó×Ó?Æ­la:z?àTãtLý?Ô«œD£C?Ƽ"W'?Ð<Bz"?±[My+V:?¾Ë6úݚ?è%ïÄ­ð?ÑMxYô?ÉQ˱zÇ?°àI+>žo?ÊÄCÔÒ*=?®U­©¶*ß?âú|lÑ??µïBØÇ&Š?âs3²?Ñ$³&ôMš?¡{V™qXÛ?¸t	É?Øê.)m¶¦?ÐûNAgùU3FGL J1051.0+5332@cUŁo@KÁÆ*\}À:{ˆe"¯OÀ<ñ¨Nh¿Î%+Ž@™ÿ¯Î@﹞¿ëvTÀ*æ¿áº—âÏ}¿ïÿ)Î'V¿ÜZN>–,–UNASNone?ïÏi‡Æ·?¦²YC2›?wMP›AŠä?¦¨†€¡ì†?/½{c)h?>N¨s5ßf?曆,áã?Œ"œoð?xÀ"JÎ7?"^gԙ$	?sú^ÕD?ü?zDƒùpô-?î¸Ê-Fµ?"¶d¶?"—×ú)7?º|_äö?"NæÇ])?ƒÚùõ'?ï_í€öq?ŽëZe‹³S?€¬Ý1žÃ?†<w¢"}‹?‡X–å.Õ?…Ä&Í ü*3FGL J1052.0+0816@n!ßzNz·@Lr)ZlÀ:{¨G²F9À;ã!"Î~~¿¦FéC\~@Í\%DÞ@ÉÇÿÞr¿ØçJÿz'¿è¤¢P¿åGrI7p¿´ÃÂV	¡UNASNone?ïœW²ƒÞ?œeÝ]ÿ?un&s¥Lé?€DŠþ~(»?|fJk³?š®›g$N?ï«NûcÇP?‹øl''?vò|gwÓã?ƒ`¸i¢y?sf椄d?yþôë0¹?íêͦ©N?štv¨—?\ªLN"?''ª¸š®þ?¢Äÿ°oCÕ?Œ½û=Üß?ïTÎE‰>c?ŽÁkû¡×?`÷_[+?j¡poðùc?"GK\ì¿è?ª£7.É;3FGL J1054.2-3123@q7KƧïž@9'¹¾ÓÀ9ëUmßÀ;³'ìüíý?ëçBXÑ9@h|	泩@ÀÚñŒö¿ãFBÂGbÀ¿ëSVÞÖ\¿ç҆²X¤©¿ïþçSá©~UNASNone?ïÊ£í^ö?€ò0¦œ®?c £$ÍëA?b×^ÆÆi?q·¾‰?}t@(ÿb?ì÷Fz%b?¯œDÈwSý?°¡Ø(߃?§BA"ÿí?ž'É\Õ¤?Ÿóaû")?îÕâ5%?œ½AJ'%?¡oÊspõÄ?'…´qR2?œÅ®Òybs?Èÿ½dus?çÊð.ã[?²­š;®ªÌ?ĬL#…6?­–ƒõ4y½?¸Và7~¸¶?©z{Љ"J3FGL J1054.7-6006@r
£Âˆ¿Ý'l¡"ãøÀ8…æ<à[À:7 Wù¼?æ¿M:ö@
Æ`Â7{@i³ +9?ï÷‡'að>¿êò1¡°¿å±ÊsbοáÉZ
§<´UNASNone?"×[X·Öh?›'±%îç?›à5¸½å¥?¥'}'5t_?îzCwtR?­Tϯ­?ˆ?—ëbè†?©Cnóò"?¬ù2ð.Ú?±X¹Tà"Œ?íwՄ™¼G?·ûô	`]‡?ÁLuH"F?§Ød
?Á·¤ûx½5?ª+ɃQÇo?çKC£Ï¯¢?±]ä
×CÁ?ÁwBïjù¦?µr¨R7ª0?¡JÑ?J¾?žÝŸU.B×?êˆZ—Lê?¸ »óåWµ3FGL J1057.6-4051@qŒ¨$x@1ÙUmÀ:yߙX+:À;Äîð
Cµ?äQSzW#@
êÖxF?ü#Ÿ—_ƒ¿ç	­³ø¿âkrÐé"T¿¿}t$¿þ¿ÁÁZà˜¨ûUNASNone?ïãóä¿~?'Þt'Vàx?;ßLŽŽ8Á?<~<?s¾?h1®°y?'ØŒ&¼.«?ï›ÇÄ~œÖ?'þqVýo?lIà`J(o?oÂz!;Ç¿?û–ÈF@\?Žâ |<d?ï1*y¤Í,?ƒr'Ч?Üùû#?rݜÁT‹?ìhNÞÜ÷?}}M«YßN?ï1ñ²ño?'	µ¤óè]?V–'/bÇ?jý¹mŽÛ:?˜^)~Ûç?pk‹àm43FGL J1057.7-6624@r>1[W>«À}'ÔÀ9«'!üÀ;<©Ôz@?Éþ"7ëÝ<@.®oês§@­-êñÑ¿ãG=Çå:¿êÌj¯ÔÌÿ¿Ö—¿s5W¿âÛמ%ß'UNASNone?ê:!'?Á¬ruò?‹‰›¬k…?–•ÿ)Ì?Å^âJq0¯?ÂøI÷B;¥?áÃü¤"?Ϭz¢¶?¸•mÿþÂI?µÆ‡j?e?ÖTŽVH?Ê»_°y€Ô?èf«ZCu?°ÝpQ¾ç?«5Ù0Žh?—.@0ÉÒ?ǗÜJÐ,(?®?]e9Oõ?ßë]Ò&~Ž?¾Wó½W/w?›/Ha¸?™Ò©ÃM2¾?Þa°ÌÔûV?¿$
SJ3FGL J1058.5-6106c@rœwškQ¿ò¨´wkÀ9&5îþÀ:HDK‰kN?ô—–"×h@E¬5¨ƒl@BÁf½y¿çZÙÀ¿ëûÑD¿ÝAåu´œ¿â_¥&À‰UNASNone0?'Ć_žpw?›U
áP+æ?ҋz?œÝŒÆúƒz?îõ—Ì»ÂN?§uŒ¹Tb?¿¨¸hÀå˜?ÅóڍÀ9Ý?ÁoP+ø£F?ÄíµÀÒ¥ö?ç¯çéº{?Í5Egs"?Åà"o"ÃV?«…âxßqŽ?Ä R"P79?«/Q?åƃ\?³JÈý)þ?Ðð;ê'?Æ¥•JÐ?™^Ìðý³?¢¢{ñ/ž:?æ¼ìî?Æåj	=‡3FGL J1059.3+0224@oY4Â@Jį¢ðZqÀ9˜ô¯úÀ;L"ø?Ûh_¤D1L@ªæÂAX@ÐßÀ‹¿´1]¥Í"ƒ¿ä¬ùAc¼W¿æÂ!=ƒ`¿é§"ü»kÀUNASNone?íȆ‰~þ?°=
™"{?¬å€N0h#?®eJdón?ŠH~$Þ ?¹†¤j?ï0âЀc?–VWKF?˜¡º{jU?'3æ@H?"`e'd|Ã?…+ÅÝuP?ì<øÊpШ?¦«rÝÛë?°Öi_etd? cããµ?ªƒ š(°?—	w|«5u?é"0¹ á?®)Oè¤?´ßRPé?£zø?ÁzFÒûƒ?«[T(./3FGL J1100.2-2044@pë•a'@A‰°¢ÊšÃÀ:H–ÂNĉÀ;Öu¼D¿M¿ï-Y[ÇO@þ\¿sÜ@MÅ¿g^‰¿íF½K¿É€tR8S¿ëA¤4Óp¿ÜdÌFÚUNASNone?ïÀG©ÁN?‡Ô°æð@?~È[Bz?‡‡ðˆ2Ç?>Y<ýÍæH?@Ûyì€O?ïÁÞYò#?Âãˆ
Å,?jþ|
w¸?p"{@?q'»ÍËhL?u‰†e—þ»?î­áûÁP?"ÁLE¶c-?—ƒ6˜nþ?A‹0à}?'Üm'úfô?&¾¾ 
?ﻧvËQå?x×Ã"ü€¦?Rû·tÄá?[¿·2xó?}mVÓùÜ?wg·6Ö:_3FGL J1101.3-6032@r²-V¿àS.øî¿À94íbnŠ!À:lÞÁÁÖпÓØe—^€ê@
°Øù‡Á?ÿu˾Úƶ?ïá…ï¡@¶¿éᖸ52‰¿âV?Zf†¿ça
˜¥UNASNone?°YhÜÔD×?µÓÕ
ÿÝ?ogŠc­˜L?sˆ· ×z ?íÕkZÉÍ?¶U]Êm©<?ª~RÅBü?»Ø¾u·,%?Ÿ–Y‹0±v?¤Û»''À´?í[hº&E?¾¹'uᶃ?эÊGíwõ?³âͳ8´?³¶°ÐS(Ï? ~`NIíÅ?äÂDÁþÞì?µ»ZnËa?Ö֑"bö?Ä՘ÕÏY/?vZð£v ô?s ݜ'Ç%?äh³aD?Äî4‡úy)3FGL J1103.3+5239@c93Úøßz@LÀ!ÀD(NÀ:At™/À<¼²£V¿¿iòC÷%@µMBs@ñç_u0"¿à"°¦Ùý¿ê-	ﻐ¿åSÅÀÐ%ƒ¿ïþ'ÝQn!UNASNone?ïô\0*…?•ûםSÆê?RÁÔWÁÁ?•üE*O™?2-Q"Ï?5ÊÜoëv?ï?.<®Æ?"Ïë±#go?Œ–gAh=¨?ø¶Ä¬²1?ƒž	'æ@a?ƒä,¿Dû?ï¿ýT
?-}ÐÉ?'(!òI""?‡
[à¾W?‰ÿ¼Æk?}°ÞûÍ?îÅÛ	¶??™,‰"m(Ã?'þ®=ÚDu??Ë.·Y?•EðŸ®ó¤?'Wi°÷õ53FGL J1104.3-7736c@r'—CécÜÀ/é‰XÙµéÀ9ul¡
ŸÀ;Qý¢W®=?ïd»þ8@O¥ 
Œv@_y5¿Ôpͼ¥§¿éM­TXê¿å_Xœ"ü¿ïÿGã<¦UNASNone!?ìsV@ÍŠ?·‰x¡W?±‡"Ãÿ¿?²j˜·mŒ™?¥¼|˧—Ý?¥›{²|ހ?ã>Xv?ÇûxÇc"Í?Τ&ž?ÁA³qí%?ÅVà‹ÿ†Š?½)6ë5¸Ë?æË`ËT¯?²	ƞÖf?ƬÍF?¬/Y+a?¼KÛk?À?¢¡uޞMÉ?ٙ;"âô?¯µàé@
°?Ò#±m=ƒ?²ZནèC?ÔCb
߉?°KTµq
3FGL J1105.7+4427@dÕô!-w@OSS&ÂÀ:Ž=EíÀ<;tÈ)¿³"š²@
Îò+Öó@>Û_· –¿ã[ºæÆH¿æqrð§6T¿ä,OÖÏQ"¿à}J$þUNASNone?ïcÄÞ F?ªi1[`?ÚÁ:TCÞ?©»P>t‹l?lÐv«²?qRZaÌ?îöm…ŠÊ?¦±µ0ì˜K?"é~®c?  4·)?Š'"rP¢?"ƒèw©?íü»òßܦ?œd؏øý?šM÷A¤ÒÛ?•Ö>R`Ü?£
E1/Ì1?~ÃÆÎ1?í½˜£%?¤±ëê&?Ÿ²º…6Û§?.c>%'¬?¤V13Ú_Ý?›¬Êÿ7M3FGL J1106.6-1744@pçquŽ!–@C7-À:BHû"±À;¿~6fÄZ?õòs´@
2"a¤
@Bÿ¢7"?îmÇÆJ)¿Ð÷–±Õ¿ádZäªm¿ïäÈQ'ÃUNASNone?Èç°fØ<'?ÅΖn™Ù3?éòš?Æ÷êûÆ"?—Á~†ÊÚY?¡tŽ(Û8\?¸Þ½?Áµ"uôI)?ërð!<I?Ä-j1}¦?¨"A².ô?­^k³eB?Ìiå#ò°`?³Š§1˜»?勳;–÷™?¶­µ3á?ºÎ›Ûbâ|?¦q+[؜'?½tԃ?Â?²WÞL•'r?êß<L6D?·«8~©Š?§"'6wÄ?£/ôU<A~3FGL J1112.1+0500@orÓEŒÒ@LÎéd8À:T…òó¨À;À°',ãŽÀç§íå@:jôºL@¾ó ¡Ë?êÿßfWwá¿âóq@"õ¿èj~‹¿ÍRU`7UàUNASNone?ïç9<èöC?kvéaµ9?^r2Úäà?cíUG%øç?ST8•%?YkõLã«?ïØ|ÒsÄ?x'ÊU'Úa?b!ÒLº?m-}³'Æà?eÞi[@~?mՅ‡M§?îD_Ñ/hÈ?™˜c*Å.«?›ÂÌü?a?'[:iÍÍ6?›±8ÝӅu?‰#ònå?ïå3¿ÈŽ?r>ÇùW'>é	Ð[W?"êêïí?j³1-®V	?r6­ûZ83FGL J1112.1+1034@noY_í¦a@N¯hð"aúÀ:TËf›@À;Ë
Yö›¿´® HC@
ÙùXqQ@á'À8iÔ¿åK/99‰¿ì}0ÂÀ"j¿éÊãÙâ<©?áb$•ê;UNASNone?ï°¡ØZ71?ŠŸÒ}@V¦?`¢ùýZÚ>?cQAk
øï?]–Ô6ú­?‡÷fF»kM?ïĈɬ'Ë?‡©yvYÒ?lèGòGá?}Œ ·Q]Ú?nŽîa&-?x¸"ß´ø?î/.Še"#?•ÃQ:³3¤?'}q_5Î.?"çfë}a×?£Î^ªÖ°?ÃmU¢'?ïÆç5Pâ¤?€wa·$l[?3¿€Ðoð?Jÿ'â=±†?{PmJŒÆÞ?€I¨ÅÐ&Ä3FGL J1113.1-4515@qÕ¢£Y6@,z2	g‡ÏÀ:)ÆäUŽÀ;†N']‹?Í
Gö'¨Õ@
§ÍÓËD@–«ß—TÆ¿è2Ùhˆ÷Ø¿âÏnhF¿äT®€¨Ô¿å7&@l½ÕUNASNone?큓²u?µÆ"øˆQ?'ôxk/A?•Ù1fqÆ?®ì3¯A?³ôzÊåƒj?îpžÄ]?«FDPî†?Œ²®kh:?¬
êMûð?¡Ñ¢ûO`?¦ã–ÒË\Ç?í¹ÅôTZ?œ£Ò´zN?—r›BxÜP?‡rX#3-?¨ªSü7?–OÖÔ$‹?ìý¶ibÚ?£Â½®ØÓ?•ô¼k5Ö?Œò¥¥â?¹òã1çs¦?¡ŽÛпq3FGL J1115.0-0701@p'Â;yRÒ@HQt>–=ÅÀ9²!gXÔ­À;¥¥
æãÏÀóEâ¸Fƒ@ÛÄÞ@è~@ÞR 3Q;¿â¥ç*úˆ%¿äʑ5òÖ!¿ÛH´ª>†¿â§¡²AÜUNASNone?ïýÉu9iØ?*£=Œ!›Ž>ü[3#šÕ·>ø^øö'?/ÝFï.?)/·IÄ*?ïÕFòdæ?|$žÅ©ÏÔ?d[ŽJb?tÒ
ÉÇ?f^ώV?mÄg°¹Z?øI1´?vYç8Ïñ?jLž#.?]z!âpG`?'ŒF*Ǘ?sznT^@ã?ïöQ±n?W'X<ñEÑ>·,KùBO>Ùß!üL«Ü?SVÒ¾ÈÔð?WŽðþ³3FGL J1116.7-4854@qõ>"åÞ@&)÷LsÀ9ÑûÊçÀ;veŒKÓ=?壪¬2ð»@—k0O©@­J 4¨Ô¿ã°ÝŒ§\•¿ç·ó…âòB¿ê&µ×›e¿á³
¶w½UNASNone?ï¸ '?ÎVëe?i'fbÝq?nálåã ¨?w:¼ÁýòŽ?}›¤O҇?îXßû?°Á­·Âö?"µE[—E?s{AlÕ?¥Qý®ø:7?¬rvHF®?î£I2S²8?"Çå]¦ª?ˆ¦¿ˆìf?|üß|›?ŸCyñjJ?'iþ˓á±?í?Á·Oü?¡§)›çâ?9Ñ»Úê?=Q\í;³?±ó}Ø~Ij? 8w""—A3FGL J1117.2-5338@r,\ý
@¸èBt×À9_Çȁ
²À;aHZ⤥?ϟNéÆO@Ô>¢ýñ]@uÿ‹í¿å2. ­R<¿Ü<
"¦¿ÓÒ×CÚ['¿â]֘[3¶UNASNone?ïòíûéc?^V Ç|˜?1
N¯ù9¢?+{`Ꮸ?Uát;}‰?\õ(iI?íEà»Ïì?¶aõlã'¸?xOõµrru?zØ+Ÿâ'µ?´LÊY{?µ¶ä-]I?îønäJC?Ö¦úŒaã?ƒ$¼,4Jß?y¹
½‹t-?—lÔ
\'-?‰ÿÃLTi?îã˜Î¼ñ¤?nr˜Ø?Uµº§ó?V Sñ±'z?¡kS"?0ÐmãÚ3FGL J1117.7+0217@p
Ô`ªdÃ@LDêòRÀ:0ªRNmÀ;ʤŠŽcÛ?××2lõÝÎ@îáI±z@9è_ÐJ0¿ÂOØÊã¿äÙGdÌ¿ä"ùiÓÈ¿ßþA†TÇUNASNone?ïðí}ë¢?_UOm/—?J¶0Œ:?P`Å¢Yÿ?R¾ŸÉ?WI|–½Ü?ï³X®¥9‡?î ¦5?s»íÆm¶F?xÛ?@{%»?r—ºæõ…é?tp©?ï{eÛÇ?‰èfTÌ?‰wvGƾ?,q¼áp?ØAc:e?~´ãOx?ïôPPDÍ?']}Maj"?y¥Ð‰=?vnàe?—ÜÓ"*?'
3iÄLî3FGL J1119.8-2647@qmMüã@?ÂÚ/­mÀ:j<?KojÀ;ñÅ	‰ì¿ÆÔ_ï @ì;›ât)?ýSwê"¿í\B_[ö¿æ&+7]±®?ÙûHñÓ¿ãZG'öjUNASNone?ïûnޟ¾!?M.Y·,Ï?L½/.ëà?MÍöo—Ü?>uÛ¶C=?J«!ÅÉ'A?ïƖ@)>'?|ýaRV?h0ú÷^ä?jÖèvv5?pœÞmå<ç?u/ÿý›b?ï"gPd]L?zïÇÅ?qÌcLj°?iÌ×zƌD?'—ŵè¿?rnÒw×[Å?ï°µÏp?"g
Âçþ?'	ÛäÜ?+&^-X}?ƒÎåˆ+ì:?"[LÛÒD3FGL J1123.3-2529@qpö@c^@@¡˜¿pÀ:$€èȬÀ;ȯf•¿«¬"'µþ@kÚÔ¢Y1@Líõ®˜?ë+Uæïì¿çÙi‰9²¿Ø΂‰ÝŽç¿éxuäw})UNASNone?ïR1÷F¾?–>G,?½IRÎ?Œî;³©?Š_Äå_=f?"àáB 8{?ïú£å˜?š³U©êh?'mÀR)Û?ä˜V¬›?‹À²²ãÓ?L'ꩇ*?í´AèQZ?ŸŒ±&ë"?¡<Uƒ²þ?"b½Ý?£‹÷<úT?"å⛏4?ìÖ/úSL?¬ç{éåc7?"+RSõ]?,I՝¡¹?´ƒ«˜ aÄ?ªUéß~(¸3FGL J1123.6-4558@qö5ü;Oa@,y‰7KƨÀ:1íÚcŽEÀ;šsîå%‰¿mYñäv‰@º\JØw@Žc|?ïýFýå¿à¹f™ù!%¿ë\D¸Ü³?°â×Ö¢*æUNASNone?ì¹X¢?'ý)D?uÅÎÓü\?Œ_o]Î?tDþ«¶{?~Ð0¡ï?î±!j1ð
?°N«¦ÈXý?}õ –ßf¥?'*÷…ú;U?¡/EJ‰?«è¨¨H"ÿ?ìû"[V»ø?¡¬Ò"=¦å?§ìª,{\ã?›!ëðVä¯?¨a0ã¦?"Ⴞì±?í'¼·'È?±5ÅÄa)?‰fí/¼]?•ãkpk´É?³•<¡"Þ?°D!Iº¯3FGL J1125.1-5803@r;N…3±@S¼Œã©À:RT`ªeÀ;9,G†§O?åu5¯—æD@
↏-?þw€?*¿ïìꏈý?ä<aëyÙ?™©¤/ó¿ÜêUU¿FŸUNASNone?ï—>c+Ý?'	Ò©G{C?c}]«í?hõ¨Gäó?…kÊ
P?£ŸáǙT?ì…c‰Ø?ÀÚv|ˆ`±?' ²zÓÏ?Ÿ#K#G£?·oØÀDüN?¾¯ú/ÑÇt?í$N²EÇJ?¡/ΡD4?–o|å'¿u?‡‡ùòl(?±A«4‡ÕÑ?¦ª>"6œ?ìïNí#ú?³µà/Ø?'+ÇjØd ?–&ÇڟÚa?³ú–¼1)?²"2¿'3FGL J1126.8-5001@rҝÇ%Ä@%1uÀv}5À9¢V[LÀ;Œ•ÚÈ8?â£ë#î^@
 úS˜®b@ht`O $¿èµBÙ¿àÑ3cښì¿èAÌsê2¿é¨ó8hɏUNASNone?á̟‰bD?Êdtib?ÕÜ`oؾ?Èók?º*Â3/ªì?¸ÌÍÊè_?å<ϵ=RR?Éry¸qñö?ÁDzÝvÕ?»¼Ûègì}?ÉÈFM‹?å?Ä<Ö]؜?êyõ]´wÎ?«PCÁcà?³MÆ®Θ? ¢´K¹º?¸âŽdCrü?¢A§ò€¼?ä:ÒÒe.ù?³³ê¢Æ÷ÿ?˪ú-"èo?²×|þM¿L?Ãiºˆ×[­?¬°W·®ßá3FGL J1129.0+3758@eõ5¨Xy>@Qf&,ºs.À9€E¯6¹ÐÀ;|išÎM?î6oùÀ©\@h¬¯Kº@N•`Nõ1¿·ÇúË¥À¿äÑ/÷®<¿áú6Æv؋¿ìuƼEÊUNASNone?Ù±Ä׏ã??Ȍaîɜi?á"N;¾Â?Ɋ™ºô9Q?ª,ðOÄùã?ªÑ¥u'Å?çúA†G£m?È*Ôu.E?ÈÃ.œÙ%³?ÅUnü?­O-(!2j?°'_®G³?と|LQ¼?¸Êęæþ:?Ò(iÖ-?¶pøž¨b&?»ÒvD½°?¢"ý˜ÌÚ?ÜÞ6?¸ÛÛlýáÊ?ÚÐÝÄÕÝ?¼VFÉ1?À£"X0?°—dPšÍ]3FGL J1130.7-7800@rª"záG®À/ 0 ±»ÏÀ9è<ʋ©íÀ;ƒÀü´ñå?ëe-žÉ¯6@½~Õ(Z?ûØ€nz\¿ï±Â¦"e?åv´@;¿¥šŒéÊîØ¿ÒùHápGçUNASNone?ïËø'H?zˆ
ßYê;?Z®ñ5?\Õ2žh±?sXl¶º?wq#:"y?ïJwùbæÇ?›LÌ,ºd?u*á/¨œ…?|,Ϲb'?'fH‡¹?—ˆG,Æ?íÚЀ÷L?žë楈?š!î-ø?mñ,sŒS?¥Br`êtE?•€bRiY?î¸úk6FÃ? Š1䬽?'P…÷\?‰‡óhÁÈ^?Ÿ¸¬'ô,?ž!7^¾Õ|3FGL J1132.0-4736@rZ¬1@*SQÞïåÀ: @‹áJÀ;´)Žnÿãê*ÍB>@±§+'¡@韍#•¿ïþž-Ò÷?ïÝ[Qy36¿à¬¤±®@ù¿æ3²UìàWUNASNone?ï¾¹Ñ4•p?"F!e­Äù?a,³÷nè=?bÜÀ|‡5?x½iýÔ
?"\:Yüæ?ëK¬…¿$Y?ąº!ž?±gí×ýC%?¹Èðí"Æ·?´:­ú	š?¹ÕPc€&(?îW˜›Bko?—#ŽÂdoÛ?—üÃd	"?'ŽÖ¿¼äÍ?¢:wê'D=?'»ø
\*É?ëÉ{ý¢…Ÿ?¾ù'ڍü?ºû'"ê‰'?¾?ƒl¶‰¡?šâ5ø'›?'ӟót'3FGL J1139.0-6244@rkî¢	ª¤¿ðZ*~…À8%ô¬å§À:…"_u±]?íä+¬3ب@·õ$YÒ@2^ÿê±d¿ÜSä,©›¿â$ËdÓûP¿ã1O¬Té¿êc€ò†UNASNone?'ùЇ?'ú ïìr?Ø (ý¼?ϙOüÈõ?ãgë!Su½?Ï¥þç'mk?C«ÙB]4Õ?_8Ì$mœÇ?àYs<¯â?ÌeÄÍŽÛ?ßCC™ÿÑ¢?Ìg›j"¿­?Å{:—w?¬;Çü+ái?Ï\ڊGdí?±Õ
m?âÉåŽæ€ç?´³9ÿ?§è#5z¶7?˜Í"!J3?Ù$)¶«?¾=FÝâ¸?áïhñœŒH?¿}ҟ©å3FGL J1142.1-6941@r\|ؙÀ}¾Ý 'À9¾±û.·À;:Æ/#Ú¿Ú®ÛÌ*K¿@ÝX›L¢@F˜ÿÀ¿ù¿ÝnŸ+:&©¿è槍çÎu¿è(Aš Ÿ¿èŸÈ,¨LUNASNone?ï"ý‰ô?¡¾2Ë¡²?v<æŒQV?{AMpÀï?š>F«»è¸? ²c—ǐ ?í¼>÷ÍA?³›ÍÅzF?'éTÿO~B??ÜÛô"&?¯"VЯLl?± Ú^ѵ?ìá²\‹0—? ¹eùN ? a¨ó
?¹™Xì¯?°ÁëÇ,ôÅ?™qE7?›?ìBAÕ?£þXˆkG?qK…ç6?iÉ@ÉÊÃB?¼Úôÿÿ	y?£§ÚJC!3FGL J1146.1-0640@q8Œ½D¦@JWe<š»À:EFšï/À;¼ì÷À?å×r%?Z@éeß­Ð?þ»È?õ8|¿îZÖ×"ø9?ÉxLÞ¼»¿Èܸûè ï¿å 5j%UNASNone?ïç<ì%˜?h™ñÉ°7™?Z› ρÕ?\Œl›¥?Vë
•	O?\¥WEœH?짪A<V÷?ºQä!
Œ?´Ma/'Ñ?¸IÐðV9U?™Õ3bÙÝ?š£¤ýś?ï
_š9?Œ>#Ô÷É*?‡·—ÂdE?|fCˆcº'?'Ä0ìýÃ?ƒªó°£uÓ?ër¨í(`?³Bþïk×]?¸ìÀG@£r?±s߇¨5?¦ûðžø·º? £´-³~3FGL J1149.1+2815@i•nÖwpz@S¤i×4/À:JÊ<ϔ'À;Ï#K^£$¿ÎþŽ]GÑ@¨¹ù¶dÖ@©¶àQcö¿ëÂ`?äO¿ã~œbC8†¿ÞôRds>ˆ¿ä®àc隟UNASNone?hžj?±uÛh8†?VR»K~¡?b~ñ¤.eœ?Œ'5®nõ¦?±ñ[¹?ïžVûWò?ŒÍs åã?t-J@)ïp?~°~DG)?|§8Ý
d?…Èÿ¸'™?î»Lç†I?'¥¤ƒ'›t?ˆg	Àª%?|5éþ÷H>?œbÞ<z.Ü?Œ}eÖì?ïJœaâÃ?ˆÉ$º`G?pä¹› N?j|Y8u?'tåE\ߙ?†ªUÌ©¥3FGL J1150.7-4816@rIø -à@*½½×fƒÃÀ:Xóz¶ƒÀ;¼ AS‡g¿Â
ÎʨÛ+@ùÔLfá@¢ÿZcN?Üù)Ƒ¹¿åՍÌÂø¿ìÛ·ÿ¾Å+¿¹Œoôág.UNASNone?í­Àríúš?Á²ç%^b?¦L_[=?³Ÿ!njžY?¯2ì$2?»ÇPª!ß?îiÄ¿ž?³ˆò–Ó"\?ƒ:çGmá?•Š3ñÀ¾?¤•b*ŸË?¯äñìy@?ìisÀ.ü?¢]øÑþî?©Ç¡wÇ?›´¥k,Ç?¯¡©[§Ù?—q7ô11?íŒxm¼?«4•ö™gg?†öúӝb?'fþœ&Ü?°½jrĔ?©¾Zà,¢Þ3FGL J1151.5+0957@pJ^~¥øM@PñŠÚ¹õZÀ:|ـ9vCÀ;âÍ)Á¿ö­sU¸`@¾_ ø@Ŝ@Ô¿ßےêË1ä¿æ)jÀúAá¿Ü¡ú¤t¿è‰¼qOUNASNone?ï͚FLþ'?ƒz"Š¼'?U†|É+?Z6¹¢?sÑ=§=,w?ý˜†'ƒ?ïÀäÝ䍛?€Fƒvº?j»,)¼+>?qás?|´?r/úøÛ\?vu/-•Î?î4.uÚ"J?•ï^ÙjN¼?"'¹=͍?…LtŒ·?¢ô<|˜?†÷À](á?ï¡áÓºŽƒ?€+º>¾?=¬Ç—Öº?BùQéŠn\?†ŸE« N?€,]³6ö&3FGL J1151.8-6108@r|Щ*0?ìʏ۪¶"À9	ï]ñLßÀ:ÒFfޏ?êZz%q9å@ðé‡B©ô@w†ß­¥¿Û?€UrD¸¿¯;!îV#<¿ë#Â2G®s¿íÔەx³×UNASNone?•'Õ{Õ(?œ	^'6Þë?뀸œÄ}?¢ºÁc¦†?¾¾ñ…ºæÉ?Áw!Zù‹?­¹°bX4Ú?¿´hëA_?Ø[ì•4ª?ÍsӔÜa?áöâ]?Ðúy¾Ð?Ï;'+­¶D?±á>‹¸3?גØ1&µ}?²b¨9‰?ØÏ^¹oa?´Š¦êì?Ɗk'ÿJ†?´Û­–¿0?ãa\Œ¨}™?Ãö`ýâ[¾?Ëð"¥^¿?»DP\ 3FGL J1155.3-1112@q˜|ßýa@H©>¢Òþ?À:ŽK†ýÀ;£1ßÈR?ð
ƒ® ¼Î@`þWN?øIúÑÃ?é#ÛΌ.f?ëšG>'ó?ç(fº¿ß/DÜRü§UNASNone?ï¸ÅÖ¦œä?")™/vÙ]?s:¯è©Æ?vjþ1?pcüÈäR?y7Úzš?쎖5DŠ?Ɣ¤©[û?¶".‹Bý?ĸP¤üpt?"…,úbÇ?¢À%:0?ì§wz&Ö*?¨š,õw"?ªN(—#?bŠo)…‡?«:_Ɗ'3?ŸuUö_Š6?í»åۄÛÙ?¶õÚ½#[?¡B' ˜ª5?²Qwe˜³_?¢ÿ§˜<?¬šÝ™²Ì3FGL J1200.4+0202@q-¼U†D@Oq²•êÀ9ã£v'-•À;¸îA'šÈ?ß	袧pƒ@#æ9/w@H½§Õò¿çEÂ[H"Þ¿Õv.­3÷¡¿Ôc)ÖÖ2¿ç¼*¥ðêäUNASNone?ïß|6,¸H?o+~4Â?]s9"n??^Êð‰Ð¿ó?aÊ-´…?f"ò‡æw?ï[¸ðˆø?$›§#§1?†Ì«FÁ?†ÜÝ»Yç¼?'E¨ÅR{]?€t´À<?ïMðٞå?†q)
7¾?'Ð&…¯ž?|£›•Î§?‰ÏÝCè¨3?{š9vT€?JnG?•ßé†4¥?§¸Cs5?†ß|ü€æ?œX6S"Ä?wéÞóV3FGL J1200.9-1432@qÐVÕϪÎ@GHw…À:NÌ7«hÀ;¶­¦–Ø?Ãwx'7ûo@ø,*€\1@)«0ñ¿íŽä["ª>¿ÜI6¶† ¿ÎßÎÅ~–¿âVÎÜz"UNASNone?ïúsðRM?Dù¬´D?9Yjvx+?@:RWBÈ£?3÷"ÙW?2݀¹L?﵉Üý*?ãݔ"(Œ?tæþ[<Å?yÖNu?qfT&.P?s©<@Ô?ï=nŽºÏ?‰©‹#=ê?‡'z'òw?ƒJâèÆ?‰£ö!¿Yú?yîfu¦4æ?ï'"È2?ƒÁ`@oWS?TÑ")'»?W]ÙhÑiß?ŒávˆÏ®3?'ßjÞb63FGL J1203.9-1745@qó\=îx@EÓÊ}g3ìÀ:R·*¤yÀ;ק jٓ?éð¸Á^ã@ù½',±@ZH@5¥(?ág6s|¿Ï¡ò3Â-¿âýÕÊ2¤Ô¿ïÿ'wJUNASNone?ì'7Õㆆ?»oák_Ä?º	šã'ðØ?º'Ny–]¦?vJfÕ
¯ª?œ*—_êõe?àÈG(ÈB??Ìq?á7n?ÚDžª	²?Ì7`Y}@?­?`#3?«êóy{®?çie…"?²™eRºâÖ?É°UŒq[Ž?°ªmã'?±T,²ôt>?žZöqTG3?Ýb¡¥R€)?ÂÛwѺhý?ß/RºÇh?ÃÀÓKLX?«rÀ?•Ãl?¢,B,«q3FGL J1205.9+3315@fGohی@S›Då^³À:WÌ¥_ À;èÚ'QU?ä¿ÃôOâZ@
þƯâÜ@·9_‰¿íøÔÔy@¿ÞòÇK;¿äÕxÔ
o¿Óý™üÉrXUNASNone?ï²l	e1?™6È
¨À"?tu¹ºoÛ?…-H:/)ì?rTõ"¼wš?"¡¡7žè@?ïBÈ2=é?–‰iÛGøE?|¡JcA>?‰cØ P¨å?')}N>äÙ?+žA['æ?îFCíJ?™ÏZH–‰?—»Ú®ä_j?Zg°RŠe?¢=®wû¢?"Òÿþ•<?î|R£È)?£D‹}?›¸[hcßÈ? F"¹çT?"½R£#(?']y½õ3FGL J1206.4-7123@rµ7KƧðÀ!®ªm&tÀ9ƒ@ìYZÀ;k8$3»ï?ê'~~@%¤ÝD"/@qM éÀ¿è'½{ºÐ:¿é8úž}jJ¿åÚ´¼Dñ¿ïÿ¹ý£jUNASNone	?ê÷L÷Ûç?»°S÷C^^?¬Ú9ž$a?«ýGÖõS?¹Ø{rX—?µZýÁ-1?Ì.͌ý?Ŋ'b:¯g?ØkTy6?Äb–µ`?ÙÚ-åáˆ;?Ń5õëŽ?èÕA"~Û?¯ÍKÔÊ?À6æ™ß·?¤÷æ€ùG1?¾»Î¦¨I²?£cņ=?Øb>¥ºÈ?´HÕ‹Ã…?ÖÛFÚyj?¸2&sʚ?юæj¾y?²–lyïž3FGL J1208.0-6901@r°µ^ñýßÀíäßé	CÀ9Úe;ÃûÀ;hK!f'?ç'͌\½@
¾öJt˜@ÞÛÿo·H¿ç¦2™°?οã/žùÅ¿åÙx(¨F¿ïÿíK¥ùWUNASNone?Ø®M–""^?ɼ۱ÿñ"?Õ8uŽÙ?É	γu?Ò=RLÝË?ǞÑÀÔ>Ç?³Ç¸}†,?·܂OÐ¥?ߖg9V?ů8|·9?Ûwªâ'Hb?Å2Рݍb?æ—1ƨ¾d?°MV5c ?ò¸ÕÔo?§¯ý²Xaß?Áð€ˆ—m?¤ÝüÝ+j?ÓÆóUã-?³þ›aï¹?ÝžóPw?¼":iÜû?ϸjÛm˜¹?²ñÈ&-5ž3FGL J1209.9+7607@_Œìk΅4@D^™côÏÀ:J¹¥¨œÀ<{DD¿Ó4ƒÄ‰öþ@
§ÑjÁ?@/`œwð¿å–âcâÓ¿èësg<¿Ñ'Û ïÜ¿í>vÒçjUNASNone?î6@Œ¦ß?·"ˆ·°ñ¡? ŽNÜzÈ!?´0g6_3?üš5u"Û?¤P'V4D?<œÈj?¢¯ÁÎ>?˜Úë»!ð?™†Jâôç2?ÔŒ±VТ?•*FÒ/B?ìŸc–ν?¥g³±I?ªbj…šço?œ¸áNç#à?«§\¸,´?šfp*ôº*?ï@%Öh?•âÊ2éí¶?|Nß¾Zçu?~Ž`ÆO?˜ÄE«®y?'¸?®øs3FGL J1210.1-2742@r>ýuâ@A"–'§\ÑÀ9©±¿*À;€8YáÀÔ7cnU@ë&šž|W@¾Ç :ˆ¿ç­U™c¿ê]hÓþð6¿ØR×	Þób¿êà‡Q:UNASNone?ïþâá?@^…àK"?ÔO#­}?!ŽMî?(î™1?=7‡ªmç¢?ïÔ9F>m!?x`ªí_³?a4¤Wó¦?eÿ®òiO?j'iŸN?r°@»½é_?ï<N*§Ÿ?‰£Þûåqç?|aæÄ=Û?z9wîsYï?'U܉›Ëé?…j¦'?ïævsD?kQ¨üz!i>ÒY.Þ")>ðå /y˜?iw]$tÍ?kHp÷´ 3FGL J1211.8+6413@`>ŒSâÖ@J.VCæÀ:Ì-–;@HÀ<3¢¾‰­¿–Ü,ïªÑ@
%›@xqû¿í¶âyÔ¤ª¿ÉƒËÒ{¿æُŒê"¿ÜœVH9UNASNone?îl"\f¿ü?´o鸾û?¨	ØúÓ&?´IgÃÐr,?bÎì
£ƒ?h‰Íù»Ç?ïzˆb"–?'΁¶N>à?ƒ¨=ŒÂt ?ŒœÅê乘?{kSÕ/Ñ?â},adf?ímŠI?£~›4a?©ÉXH/ßÃ?¢É.þ+?ž¼
¯—??Œzãï8?ïJH"ñ¿¶?BbaØ?‰äÎ$µJ?†ÌI)6D?"euk]7?iój1ž3FGL J1213.9-4412@r~Â&€@2$Wâ?$ÙÀ9›Õ¹ÛÀ;"«² Ñœ?¤63©åv@üW-
E@'§_ÕӇ¿Öaé0¨
î¿æázéÞ´¿àsHš(½¿é}œ/mxUNASNone?îâF³*Ñ?¢Y7¾»?"Á:k:¼?"I†'ou?™VŒEˆ? vÓ;ÃÏU?îæÓþëã?¡ÌwQ¶ÓÕ?ŠM`&'ªq?"ÙèÿòV
?•þÐZ®E?žvÑ¿ÚP#?í®ýiË<?Ÿeå¾['?ž(iÁFâ?¡–ygè0?¦.k"š?"½C€#¥?ìÛ.øoî%?¢xI§LÐ?Œ.—…yЦ?€N<-|?µ µKÑTÇ?¡Ç"/ÁË3FGL J1214.4-2315@r?÷eýŠÛ@Ci/Âej¾À9õÅGMƒÀ;šñ,'¦7¿ÝöECM@

ÛF["@‡Ÿœ¿äšgãq²}¿ç¨ýÀ	ÅÒ¿âB`m†žÉ¿à5\ë_×MUNASNone?î‹Ç¤ÑEÝ?¬ºwT†?sN#zwÀÁ?zfå' ?¤ÙÁCœª?«g#_=z?ï|®kdå?'Mô8ÅEŒ?€w/7& ¶?†


?€ƒ%.&?†óâfšÍ?íÜøú"¹ã?œ>2mcºj?'šÍp¸?Œ WñÊ?¨ï¢ðø?—M«®Fj?î<çFɉd?—@llªÃ?k7ËöÀ??hÀVþqã¬?ª˜§ý¤?–ÀŸÌý¹3FGL J1215.9-1926@r8Œ?>q@ES3"l;'À:-H*;<íÀ;ºêßÝJÉÀaa;.T@—ÿÀ@Pwߊ"™¿éßv\›¿ãñ¨‹Üë¿Û€Sɱ¿í;=ž¤£ìUNASNone?îö5{Eñ;? s¨¬gì?›ñ[ö?àÝ29\'?x™}ï›.?Q­á8?ï˜WÖ)?"w°(cSÏ?y#é{8F0?‡ à‹?z°ˆ³,ß?†H‡Î‹¬?ëþËíJç)?§@ل‡ðW?°Ty(s?ž˜"ŸÈÇ+?¯k3
_<€?œ³ƒŠ]?5?ïcӍ@?"D¬wùóz?:Ù╗?"?Wþ'*zù"?"&Ÿ3?"Ý°¶X˜3FGL J1216.6-0557@qö8<òϖ@Kí@$³=°À:o®
ÅÀ;—\>Å7­?Í,Xæ˜ð@ü;û-Þ@Ý0ŸÚü:¿ç½žÁ¡ y¿ä°ÎøSÁÒ¿ãu7	àC¿ïýÌn®'UNASNone?ïОÅfÑ/?v&à¸àÀH?e/Ê>¤X?f:åJþ?j1p'ð-?p*é?H?îú(ÐN>h?š~-©?"Ž[ó`é'?"f­åõw?ˆY®"˜?‡ÿ¡åBì?î"__†*?˜ìôBŒÝõ?Ÿ· 1X^²?ˆ†`v²?sâ¶Ü?ŒýÈBŠ\?ìtÍ`˜¸T?¥€c!¸¦–?©=#äÏå·?EÂvY?¯v¤•?œ^
§ÐÜ3FGL J1220.0-2502@r_ÍÓØ@B¤!ÀD(NÀ:WfÛl7À;¬—AЄ迶
ˆnÚñV@ŠJ}Qº]@r`Æ%¿ïÆ»y$?ÜÎk6Ʉˆ¿è>)YÉ(¿ÒÈ*Ïj£UNASNone?ïà~b`l?wåWx¿½n?h!úüX?os5û¨³7?OCÅî'_=?q6ÙÎ^¥?ï»
òÑ ?'(ƒ+pú;?p‡¿Ná—x?x4sâ®[–?qò9·µØ|?u¬MŽ	‰&?îî}îám? %°%?'R¹TýÎy?‡‹]¾2"?ÝˆÎßcù?€)»Â
M?Øhìb?…ŽÀ›è:ì?w|‹~À¢?}&
¢›?€K †ö?~·xK.œª3FGL J1220.1-3715@rAc@93MjOÀ:š¿3‡À;½ò×"'%¿ÎDn?´Üý@
ää~`y@_ßÿY'í?Þu`ZÄØÉ¿á· "IÖä¿â€BÌ=¿Í]ßØ\UNASNone?ïÊ]·ŒZ?Žì͂|4?Z#V»zu´?cÉ4"Ø"?w±ûu[5ˆ?~JÜüØ«~?ï¹Obu\+?'Q-wS?kXILÅß?l WVFwý?u¬*
?|v¬O¯=O?îÂy´ôØV?Žç#Ák?(%-?ró¼á
?—›¡O?È.?ƒdgA‡jc?ïy/#‡Õ?"'Ãr ÿg?X¸ÊúB%\?`bºÚc?šåMkêâó?"7¹²ò;e3FGL J1220.3+6055@`4'¾‹Áj@Kå~ºñ6À:ņè¼í\À<  ‡Êd=?¼"Ze@9»n€'@#?¥‡d¿åùáéû˜¿éÙ¼06Bv¿ìv'"×?âK˜N­kUNASNone?ïZ	Ð<ÿª?°.†"Ùh?"/ªñYÌ+?°%ÝzENo?Xñ°pcéÖ?aŒ›'#BÃ?ïß·Wc3?…¬‰ÊÄú?o&À›QÛ?|›ì#ÎG?m9ˆ
KÉR?tÊÛ¥!ÔÜ?îiÿd+*ö?›51Ý,ªÈ?ž¦v®öÿ?™Mº±óª?"¿mëªJ?'ªÉ–?ïç*+{À,?q!Æ.YE˜?0ÜO'.‡ˆ?G6;8ÀÁZ?fºJ'Ð?p¯X$ÊOl3FGL J1221.5-0632@ri$ò'Ð@KÆ YžØÀ9b+åaIÀ;'ÍDÁÐð?æöËA˜Œå@±VPÇ!@ÿ"_mλ¿Ý-V·$x¿ßìj…ôù¿áû`Þè]¿îÍ¡¸ÄN›UNASNone?ázi2–N?Çì2âžè?ÛQ…þ®©?È;ùOL	¤?›šyÍ#«Ë?šù
"¬¦?æl­ÒáB?ÉNæm¾Ü%?ω3½
ø?ÇcAJû[?«V†÷²,?ª]sÆyÝ?å:P
mSW?µžúýö9?ÐÍxái?³ÝCÎ98?²÷œM¥?š6`]~¼6?ãW]©C€<?»‹9ÖÁ
=?Ó5å(fË?¼¢##j2?¸m~MBbî?©U€µÕÁ™3FGL J1222.7+7952@_ Ò
ú/@B–-û¹À:Â3|.NÈÀ<%K#É¿è}ê!Ø~@ÅXlþ†?ûËÓÀ±ád?ïî·JÚnÌ¿Ü&¢¡U$Ë¿ßrøËXX‡¿¼ÖçzDŒUNASNone?ïâ,=†±‰?¦Q<~ì:<?hÅt‡¯C"?¦O1b?D97Æ|Ì?HÌaI¼×?ïÎ@"¤¬?{ӅK;YJ?dºŠüºX?jۑÆ{ûM?mð^™Í?u}˜ÙžÀ?ï=€áì?‹®Ä4qów?òÞ¹?"ýîe"IX?Ž¬èÿ?#?{ɒ±þ?ïÖ…ó£'?tˆ¡àG6?:ÔÙÆÇ?$!CÖ?tžQ²Ç'?tfWôÿ?\3FGL J1223.0-5622@r¯®]á\§@Š\å´$À9_7T*#ÀÀ;AiÂ;yS?è~Õp_c"@"üÄâ@4Ô@®¥¿ç£Äë¬â¿ç7Ì@\¿ìð³'ÎêοçG¾É1•WUNASNone	?é>~EYì¤?Áö8ÜQÝ?¼þ˜Æà±å?¸£dö†øj?¹
uOé?¸ þ­?ä±ÆÑ­j?Í{èxÍæÇ?¹Ë¹Tüî?ºKŽX˜?Ð)"ì´?ÈCY 
§¬?êóKË‹?ª÷T^?®$‰Éû#?—µ5`¯'?¿þ!B6?¥‡D̑21?Û"ÍâÊ{?¼$HÎ&LÐ?ÒíEÌKáT?•þABHÚ?ÑïìQ«T1?¹Z:Fœw3FGL J1223.2+1215@qY ¥&•–@Rn•¿ðExÀ:Uÿ'E7BÀ;Ôzª3?âæêÖUÀ/@
^)Òâ:@´ƒàtÊW¿ë¸Kwn¿šº"|È¿ãÆÔ²–¸¿êjx"nëUNASNone?íS$=ê?²¡(?øáÊ?±¹ÐäH–n?°³Ãlâ<?p¯Î@ÆÉ?–(AW¤í?ëÀ8CJÀ€?Áb$_%ËÄ?¸žqÏOÑ?½ä™"h'£?£ã>çµX`?¨…HËÜ?ì9ьԏ?§?À:¼Ç?±âÕÖ"ü?¢#íÌSW?¨©`q?–aÒæV£?å7âJnF?ºfkáÎÄ?ÓYæum̦?º ¨
1©?¡²§­±?—'ÎÝ-¶Y3FGL J1223.3+0818@q¢éxÔýô@Q'êžnëpÀ::H=†sLÀ;ËÿwD?áP½R¡Û@
÷Ú·R?ÿÁìžú+«¿å6l³)(¿Ä¨M ‹•¿Îy¨çH¿ë÷4£[ö\UNASNone?í "xT0?´ºQ<•?²daÜrQà?²ú6Ï%?'j)ƒµò‰?—·:»5Ü?ëÆf°ÔF?Ã÷*äÓY¦?¸•'§Cь?Á Vø¸Æ÷?¢t´Fkœ?§M°é_C?ê߄uus?¯Ïúº¦Ýo?À ±»N±®?«ÆÿC…y+?«@Ëmâ/?™§PÙ ?몯½èLh?²ñ~3Ëì'?·Ë–àì?±D?%Uþ?¥½âóº5œ?h:Ã3FGL J1225.4-3448@rŽg ù	l@;†ƒ<`À:ºèÊYUÀ;á'o°'¿ô±ó:ß¿@1PÊÈ»›?ü'ºž÷Ò_¿Ö25ÿ¶¯¿É3Yö¸Ðä¿ß­[ÿkl?»}ÙI²ÑyUNASNone?ïñ'£#s?Sñï´O'`?L—§OCš³?K¼Õ¥Xº¨?M$N$.›;?I/ä\Hg?ïÏõèµuŒ?zà£Ì`Õ?b'µ"fž?gFt>x?m‡b(#Õð?t–#
ÈT1?îÞ&'Þwz?‹¶B¸¶H?76oN??ƒVûQwEÒ?"÷5%Âo?€0ùYùv?ïãý!úØ?gü0·>ýÿg¹¨ôG?ú9™îs¬?kÆß6ŠÖ3?gêƒÝ3FGL J1228.4-0317@r;jžnëp@M‰‹ÖbwÄÀ:ìÝäLEÀ;¯
õ´MÀ£$u«'á@‹ÝËø'@,û GH>¿Ìˆ©'
.,¿á™âGeù¿ßX#¦ô¿åôŽï`d^UNASNone?ïÖ[Nh+:?œáÿ0ƒ?fA<ÿ;??"ývgÄ ?cct˜™†Á?'aG™síÖ?ïÜji¤?v2n]­Ð?]É^ã}®?hoVÖ_»?d°æê#a²?nssÊm©?î¬'ˆ—?".{ÎZ'?"ºdx	{?‰ÿD/ñfO?–Àª`eãÂ?…gÇC!"?ïø•«,oó?hiÞV>¸Ü±ÈÖz>ý/'Ï;M?Mœäõ[ÉV?hô‡$_3FGL J1231.6+4825@`{ԕ*™@Q`þG™À:Ø£š¤À;»‡Ý¯s ¿º'÷‡
¡@WÀ<pž¤@À‰G'¿å&ËEä¿åV c€`–¿ëQšfÜó¿ÛGÎûü[UNASNone?ïÃþgÌ?‡Z¹6Þ{?jE¬ü
öè?r›V‡A?pÝõô}^?výæU=½±?ïªGŒ(èN?ŠšGÃì"?tPñ<ò6?vš¬¼?v‹H®™¾¾?|¤Å¿E#h?îxZ!·ƒ?"¥ba8q?"'~«­?ˆ‹!•?Ø®b?Š÷YãE?îÕ¬ÐFS?—˜x±_Û?ƒ»¥"^øš?†©º$[9?›l"5
9c?"×êûbå3FGL J1231.7-6513@rÍ×süPÀqOøÃÌÀ8Ác¡ À:ôóW{?óñKle@üóʒŠÝ@e#?ö;¿àÐ9zŽÖ6¿å¥+XÚs¿èd1®ßã¿î‹ºù¥)UNASNone?§ø•Hñ‰?¤IΙdØÄ?âÌ@{1?Ê_‹lEû±?×hl`?ɧ	Ã>?‡´õÇÁ=?"Ø©\ٌ…?â~Çb¦?ÈÐ!9ÿ?ÚDÊI<ª?È%¹b•Ç8?ÍV%ÐP?°• «q'H?ÙAë™á?µ€ÈÁýÃ?ØZ~é÷?¸%†\9?Á=ìºßý!?¡Çí`1
h?á"\ɈVÛ?´Ã`\Z›?Ô8PSº?±½ˆàË3FGL J1232.3+1701@qeŒûüeA@S¾7`¿]yÀ:K1"·ºíÀ;·­AJÅ?µR"Ž49,@
» ì^¸r?ýeÀÂ}i?â÷ñó;»1¿Â½¾ßE¤¿Þ}4B@±¿Û¹'¿ÚÃRUNASNone?ïÄ*!Žì?'¯Ó˜Hñ?_­Ü	™ž?cX{EžFÐ?v'
x6#º?'æ4m´–?ï÷^'U/?,/NT'?r@Š¦"B?w+9Ëk
¨?~ÃƸÔF?Š*º¶BOÍ?îÒÈP/a1?Ž•¹ÈU/?ŽŸM‰Ó¶?€äW…o6Á?–WO5)þ®?†™ŸÂ¤°¿?îžnB{î?–ö¤Êø&,?Ž½O%Ùþ?ˆxÿ4)K?œÓ³å?"
ëa¸þ3FGL J1232.5-3720@r¬r䎊r@9`œä§´åÀ:Eä9ÐÜÀ;Ã3{W3¿ËÝ«Pj‹@#
%­c¦?þ˝_¡Ñ!¿ì¾WýJ¡—¿ÍpºZâØ0¿Ù2҇™3e¿Ô"•ziíHUNASNone?ïýIô|öŒ?2±§û¡Ûv?$™…úøj?$×V%}?o?&ǝªœ6×?(w/¼ÌY¿?ïÉdºª?|W+7Âj?e}oœ'?hQ—,éà?p·n•Ôk?umˆg`	?¹]Õ?yÉ>"Ì
(?zW§øËO?sÈM6ÌA?~gûz?jÓvëÜ^ú?ïÅÖ0Y‰?rÏÝËb?0óC{#Bå?4à",	áÖ?|³Æ!i?r~L"æ¿*3FGL J1232.8+1332@qÅ)ûçl‹@RîÐ=š•BÀ9þ©1½nÀ;'ÆÞOâ?֕YscÏÞ@o÷oF@]o€–hb¿ç{YŶy¿äœo
éÓ¿é{€cŠ
}¿ïþ2£nQUNASNone?ï¡-v\¤Ý?'Dt¡hôõ?}òE+àµA?ƒ|ËÝ/V"?qvÿ¥ÌÜM?Š=?/?î. {韟?­TÑZ–? o1ðN'?¢õ0?3\?™\Ðëo?¢OãϱM?íb‹gÒx"? j=î¥?¥å™=!At?"ÔW€›p?£ñ°E·<j?"â€nÒ?æN
v!?¹±¥à6‰,?Ì8c1·4e?ºd3ì?µÍëÀŽŽ?¤gçÞ.Þ	3FGL J1234.7-0437@rqe"¯O@LÿŠC»@³À:ŠE{4SÅÀ;³"¢Ù´?Ùôÿ­@êI5Ó÷c?úb¿?›vi¿ïÕ@–?"b?åÝÝ*_qw¿ìõêÚBÅç?è\k˜ÕN|UNASNone?ïÖübq?|ûŒáFß?r9¿Ô¡?|/6ZàN?C|©—–î¼?JIИí{O?ïҔÝÃþƒ?z£œS}þ?ft;£i?r:b©/W˜?f÷^??mÚêÏ ?îÁå¦C¢Ä?"ue*ú(?—…Ü5?'ydz;Ç?¤­²~ËT?'ÁN79?ïßLâŒó? 'BÒA?\zy?ÚK?xÝ¿ªJ?bv¶l÷Œ?sZN¥ðoÜ3FGL J1236.5-6154@rÒЛùÆ*?íSó.ZÀ93»ËóˆùÀ:Ÿlç‰çu?ȐÝ,Y›@Ø+Ú#w@ð¸`Y1¿è­ˆÖËÆ¿ã-\òÓô¿é½)Æo\ü¿áI踪oÄUNASNone?ârbé±5¤?É·ø€"ûû?»Ä'À2?¹‹¶8+ÚY?Ô*0Hmˆ1?É@ rÖ0[?ÀUwš'‡o?Ç®–Sl\?¤­NFÜ?ªç€{ý¤?ꪁ^†¹¶?ȯ$A¹
õ?ݓÏ=ˆ†?¹Óx
UH?Ä+YØô?®'ñí¤8?ØV¢p‹?·k¶MܐÃ?æ]óÑ<D7?¿«Ù?Ç÷ç‹?'VUÌXSL?ҵإx;7?¿%ˆa½3FGL J1236.6-7050@rÛMžƒä&À *™0¾À9Ôÿ¢³õÀ;dÎ#"¿îÎ2c»¢i@ß	»?²@©c `Ș?íM³ØØ¿ä##À›Þe¿ærQ2;€N¿ÝÒ"…¶¹UNASNone?ï5ã
L®?‹»ßw>íæ?h"º©(¦?p¼DÞBdµ?†€Š7?ˆm¦'8«?î"/'#?°a
d³?sq_E˜?Ÿ?'wY"ó±:?¥NÚîKõä?­6č}V™?í¦¼ß,Ô?™p¹¼?
‰0¥ÜÃ?Š¹oå);?§íuêD^?'ô%P>É­?î€ÿܹ]µ?ŸÑaI>Á~?D™ÓèE?KdÚè?§Ÿ"̓š?ŸªDÜ#3FGL J1239.1-1158@r£6âë@IdÿñÀ9­Öû#ø-À;"ÙHÜ?ñ10N§X@D£JÈP;@ˆ ÀaŠ¿êä¿hìt¿ëäQZ)…ú¿ÞÇ\O≿å'UZPUNASNone?ï{8cÓV?'‹ÆSv?À©b&
|?'¿Z†_¾?~ø'	Ê:f?ˆCu0¦Vù?î?9ø^A=?³:H'g?¤¶dð¢?°î'¥LÅ?	T*V"9?•—óCŠ?ìc_ãY– ?¥TY6oôT?«¸–*5?›ôù-{W?®kÊ<`î?šæh?ér»¢ù!?¼$Pφã	?ºa±±?·4Oa9?º
€qå+ä?±Ù·%ðÞy3FGL J1240.3-7149@ràÝDUGÀ!ò7Š°ÈŠÀ9NÅÚjDAÀ;PPKqîZ¿ô4ÏÅЄ<@ÿ÷1Ð1±?ÿo¤?åÉ¿ç3àÃ¥v¿ãü!‡ Y
¿ÛyVÿ§PοÒíƒ~Ø«±UNASNone?ïñ!nŽ3Ú?g²Í÷ƅ~?uåçñº?¤ÄJCXï?\ą&ýÑ?gr˜ða?ï"âa²?¥˜\x¤H?eß߅cð?s¸ïH±f?šQñ"ý>?¤r ÒÝù?ï?NI=Íh?ƒåVβŸt?|Ÿ2/DtÜ?qè吼œ?îjLu5ž?=½
 ²?ï´Á"Ê)?w9Fª›ÁM>åéӒK)X>öÈÍ|:Æ?'Ê Ã(ã?w5¢"CH3FGL J1244.2-6227@rá˜ÜÛ7Ê?ÚbÅGtÀ8¹+0/sÀ:~"Ž½ž?ñZ:MƒÁ@
°(ù°@—kˆ±j?ïþßZ)Rp¿ã6âƒ~‹\¿ædæo=Ù¿ì¬wJlé@UNASNone?qþ[ï´?r	q"?ãnpù<~b?ϜõS9¸?ØÛ$Ê˜l?ϗ®&(Ï?s?ÆåéÕ®?—Iù€Ýò?Ñæ›Kµ‹Ó?ËŠÜ›…¶?ææ2ÌYfj?ˆx†žVå?´&n«Ê{Q?ž¶Ü4·Ø9?Ûø喱c?´ÊŸâó:?ß×kov¯Ç?´mOTP_?°6m¾ßۉ?¡cZ'âïe?ÙÆôtËæq?Â6nMV+L?á¸
¾V?Â<oÏW|?3FGL J1244.3-5515@rޗö+jè@gB™ØƒºÀ9_ýŠÚ¹õÀ;O¦¢–˜]¿µ\)^ŽÄ@«wÈ8"o@õò`L–¿âX´^ìÊn¿çt|')ð¿êŠ'=:%É¿âE&M¼ŸUNASNone?í«]C!Ò?¯¼ŒýfÊ?"á»È?"&å2HlÏ?«YÉ…OÚ?­GhÑ?ëY¾â#Íø?Á·ºÿ's·?Ž›»¿›¯?"¨Í\¹ä©?À·ª»´Îe?Àî›õͽ?ëæ"zï†?§z_™CÇQ?¢Œù,%€3?é÷%=S?·ˆo'qè?£…º€uï?ëo=
(DH?ªþfªí;£?É&Ê»?Œ6|c‡ž?ÀFyj¾".?ª<Ɩ'
3FGL J1249.1-2808@rå2a|Ú@A\ÚãæÄÆÀ9Ý68¡1>À;ªíñ	Â÷¿ç•ÿø€§@E
6ÊA'@ˆ‹`pÙ¿èÛÃoMb+¿ß)ŸÑ`I¿Ýj…ÿLÀ'¿ÞŽk›¸
UNASNone?ïäI%¹J?u^f´-ؚ?I$ÓÃ,‰5?W'j$MèÇ?em¥UêƲ?qmHH)k?ïÅQ-Zƒ¥?zCŠŠBQ?h†6'Œ¶f?i~!M {/?qN	wÑô?s±1Ï­'d?ï^k¶å£?'jàþ¾2?{A4ƒ×Óþ?qµ­×v¤?ŠÄx6š­p?{'&Ô$­?ï—}¡–'?}x•Л?5íjޓp9?9"â•þÝ?‰q,CjÞ=?}#	F^™«3FGL J1249.5-0546@ràë…¸R@L‹fÉûÀ9óÔCédÀ;mQ¿tè¿àAg©\…<@³g€Â³@M¤`r¬?ïEcòmÆ,¿íc\›·¿ÀÁÁ‰¿è¥åÊʔ
UNASNone?ïã!Ã9ð?{x•/ˆÔû?FÞÉG'ÿW?Liß(ˆ"?g0+êáx?zM!îu?ïÂà͂†?€Ú,ìá7?n=xrmB?uQ°È£y?ná¢}‰?r}¦Dq{?îòŽ¸à&?›"›{͇?'çü??…_Eø
Í?¦õʓ}ÿƒ?—™»nC&[?î^NŒð<?¥Në™bI?PÒ=eƒ
?XDÁ謙?©"…HÙÅ?¥8\Ž8Ë93FGL J1250.2-0233@rå'¡ Ï@N'=¯÷¥À:—öÅĚÏÀ;‰Øê2¿Ô!‹ôs
@
5I¯?ñ€y¿ïôÍÁᮩ¿á Í‰¤ó¯?ç³p;Á?êX•íUNASNone?ïê»'²ã?}¦Î[x? Ÿ¶ÿ䙚?.º»ÊåÙ2?d:…
NÓÏ?}°62h?ïÖby¢¿;?y
€š¬?bxµ´§\?l6Ñ ºè?g$Ш™hµ?pïH-7ß?îl´ß'?¢îN¶1q¦?¡¦‰n›Õ"?ŸÏ3ï ^æ?™ï?Œ,bÕ?"n?Ð_…ø?ïåAm…
?w;›Û'Dg>Ñ}V˜ÌÞ?oùcyµÏ?jµÓϳõ?w<%·ˆ´3FGL J1251.0-4943@rîƒùd@*GЍK­}À9ÖBƒ2OÀ;tˆhî?á;­2Ü(é@¹ÈQ½âÏ@=ÍØã\?æ7€y%õw¿Õó(¼6Òz¿ÒÖ"¿{30¿é¡¿+é+ÂUNASNone?ëp¡¥¯Í?º5Í3»V?µVÐ$o?³B¶""å?®IÆu'ºY?¯ºéߜÙ;?ãõá¬ê#­?˅‡ž\Å?DZõgá?¿=D†ÕVž?Èvµ—8	j?ÆB¦˜ù?ë]RÂG£‹?­¯§Òèáˆ?³†Ù%9ëU?¤Äävȑ9?±ŽÈˆøF? ¤š^?å²y0>T?¸›z‹t³Ø?ÁÜN>ÖE¡?³©ÐLË?Ç[—ÜhÁ?²†±§_â*3FGL J1256.1-5703@rùHè§ç@Bæê…DxÀ97¯h¸À;Ð߁w?òùéá½)@weêÀ}´@Š<€c舿æ"ŒéC)¿è-¶G¶^2¿ëûGC,òÊ¿ì/%\…èUNASNone?ÞÞ:"RñÛ?ÇÇ÷÷ž‰?ÖO…ÆãH?Ə']d|ƒ?Å¥mëÌU»?À&9- "?Ûó'kìóœ?Í£ø¦gg7?É3Z4'[?ÂmÞgah?×rôføÃ7?É÷_À´¹-?á÷Mø%d?µ·Zéƃ
?ÐÁÓò¢ZE?±¢X¼œm?Ɵ :'Eá?©bÂÜ?Ёs0¤·?´CõC?Ý€jÛý?ÀÏj¿DýË?ÒgeÎM?¶¶¸Ñ¹Ç3FGL J1257.0-6338@røт©"¿è¨À~	ñÀ85«³w'À:‡/	ØÆÖ¿¤8Î@ˆr@ÿqŒ_Ig@ò]Àz"¿ìÞ—ÈšI¿ÂBfÊíØ¿âGŗé¿éY˜ÖëUNASNone?ìv÷܃žì?¹Zp‡-?Ÿº´Œ<?¤‰oK?´YÀ.¿ù§?µÝ;²©ZÏ?áñcTd9?Öå²9?Ÿª¹Ã>™"?­_œIY?Ú##Mö?ÕO
âXKà?áqî½­7¬?·~°Ã³gÁ?¹C!HÜAN?¥p^!Á¢?ÖËZ2n€V?¶a;æ—.?ìÞÿèÝ¢V?¬uà30™C?c…'²í^?d5U]ÎÝ[?¸k×{{"Û?¬-cEšIà3FGL J1258.4+2123@sî˒:*@Ur\=îxÀ:1—¿¤ÆÀ;'UÙPhÎ?ñ[Õcõ@%ÅäêÑ@&K_yã¿ë¾Î×û¿ïÿÕÝÚ?ïýåu²¿ä§B"èe7UNASNone?î¶Í)Æ°)?¸Q'i¹|R?yz•Ãv"Á?ýyصp¾?¡cÚ«&*å?·UÀÉ?îð² ÿÚ?·ÕoÖóú?"åå¿Ç;?³Øþ¬?ŒŒ@€£^?Ÿag<)KÜ?ë('@Òë?«—¦f	À?¬Ñ`¡7~*?›íïLF?¸RŨÌèÉ?¤ü·RM?íú!±Nz?¹!ôT®n?y¿g\ʈf?žo7²F<Î?­'ðùQÇR?¸IÕM;p3FGL J1259.3-8151@ró¦">jÀ2þRv‰ÊÀ9Ê=|bQ.À;€ü‡7?âã"˜A'@Aà;i@'æÚ¿æäNò_1¿ã-=À!e"¿åSÐÄþø¿ìÁsnUNASNone?äòÔ¸'ŠH?Çþ†Óäò?É십‹ì?ÃÐ7#Iõ?ÂH!rIJò?»šêއ;2?ê®R¼"%j?¿Óâdn[‡?²»(á`?°'"¥å9?·ÒTö
ÔL?µæ_ÑÕbv?éûÝÂà´l?­Çwêñ‡·?¸=YÉwü?¡ èo‡ÄŠ?·ã¸ëä¨?¢<!wÌeÉ?åù¯tSãÒ?©ËRô±úÍ?¼±[&Ab‡?¡%Jyh?ÉÀ"›¿s?¦¢g.Ù3FGL J1259.5-3231@s™" ä@>Rb˧2ßÀ9Œ‰B37À;p—"6À
eS®þ° @{X³|@¶™ßåƒR¿éÎ]àÓ6k¿çO¶UU᣿çZaµ?¿ïÿ	̀žBUNASNone?ïïx܁ F?d•>àx?Xñ÷àþ·ò?aÚ/½7"ª?@8ž9v0?FO'³'m×?ïÂ+3Þ?',흰û?fªÜ€î#?k¼†Îpøh?sí•¥š?~"¯Š+â?î®Û~3 ??'õT×à?–u÷¨w?‹gæaie?"®˜'‰÷…?…ºœÈ?ï9–°?'Ùml?3r&}ì?aÿsujR?‹VaLÿ?'G…ͦš3FGL J1301.5+3333@Z1ûµsë@TÍ+©ÑöÀ9þêUrùÀ;Ö5À¬-?ïôÐp‡õ@'áÂ@-g߸6é¿ØT˜Ñl‰¿áLçee›¡¿è³vH q"¿ïÿÄoAgUNASNone?é˞UöîÂ?̉
h´Ú?ÆWZ1å'?Éïðé+?–izo'ûD?·¾U@?èíŠM²±{?ÈMQŠLgA?ÃçAV:.Z?Ć`Îwúú?°Å*åös?¸Û
©?ê0û;	?­Á¬þ1?À`ë"Eñ?©YD"6=?«lŸÅ_¸?šï‰Š Ã?ßDí÷Ò?ÀkÃ}©V?ÞL'^O]É?ÁT‡¸Hd2?£t"ÍS.?ŸQc+ñ3FGL J1304.6+1200@s³ …±…@R£öÓ0"À:¬Š7&À;¾òâ
K³?ê$.Eì&@µ[©Éèl@ü[€YV³¿Ö¹®(8Ñ¿â*5è3¿î;²[ü@¿ìÂ[¹ì1UNASNone?çÄ«ËÍT?Ÿã)Aê?ÏíÏ´]A?Ū#¼ï?ð#Ïíä?s˜ßlf?ìøbY?Í?¸ùÿNX_?°îãÕ|?³Œ™ËR"? oü¥Ö(=?¥L‹æ¸W?êKŒê£!º?¬•´$É?À{'ù"jI?§¢³mÈê?©Z'o|;/?•Z×T8©?à ì€Ù0?ÂËõ9¡½˜?ÜHkLÁ9š?ė£Zþ¬S?«­ÝŒ]`3?¥Lӆi3FGL J1306.8-4031@s!° ě¦@6>]ž@ÈGÀ8ñjwmçÀ;ëÃ2X¿ò]kÑ@;®õKq@SL`UÖ ¿æ¤2
$'R¿åðÎ5úÛ¿æ2ÓD
Eÿ¿íHˆ,[UNASNone?ê¼qvýÇ?ÀjÙÛǨ?´Eíjw×f?±¥¡˜î?µÖŠYÐ:m?·©«_ŒC"?íf¦žT?¿ÅÚ*?«&£ãâ…?´_Ë¢ã»ë?£u²"83?°û÷JòÔ ?çU.qÅ®Y?°ËIè4?Á(§¿úEÙ?¥ãd£§r?Á'žxïÅ?¥™ML0?ë@‹r4N¿?· ž®'ÀØ? n¹£Sþ?ªDõƒ&ØM?½ÄGëà?²šaíAF3FGL J1308.7-5738@s4Á¨¬\@jOvÀ9`Ö@†À;"ŠfðÀ^õѨԠ@+[Àðöx@mª_åmØ¿é¡XØçÀÍ¿êöbªÅ¿ãN`5IãÏ¿å'ärʑ£UNASNone	?ì‡ÔÇÅz?½¨–G×?"š;:kJT?‹$їëþ?¹.Z†Æu?½Zð-M?íM´ì,óX?¼Yiª'Åj?~{™S´ÉK?*$îžÐ?³ªŸ	]«?º†à ·'ú?èÐØæîs?²ð‹l	?­!cs½ú?Ÿ:Ùð¥@?Å\Ôj¦´?®Ÿ'"^0Ï?ë¾Ndö??µº¿±ªÌÿ?@žÏîa­?J‰Êúùô?Àö¦ÍWI?µ³W"=˜Ž3FGL J1309.0+0347@sžoü]ö@P'`A‰7LÀ:—10#´:À;ð3PD¼?ðÄð_y@íyj¥@¯i\e¿ãS÷‡û%j¿¹U&œ"À1¿ÑÒÛ
8yT¿ïû|Ë`DUNASNone?æ—¿UÁ9?Ì9ÃL­8?ыÚúà?Ë~ý%?"_§…¦
ð?™Ïüô©¬K?ä
sTgÜj?Òn^poG?ÔQ'1ô¯b?џ‰B$I^?¬œ9)ܾ;?°hcY…=?äkÅԝMª?¶,ÓäK—?Ðå-iC³ù?´J£Ãwµ~?¹
¶ÂÑ?¢Ìø_ˆÿH?åڐR~Þx?Åv˜ŒÇMÖ?ÒA6~GË?ŖL??¡lñ$Ú.?œ"®L.[Ä3FGL J1311.8-6230@sœàuöý?ÑW«ãs,rÀ83¸"0¤À:,[Ðá."¿Ð GÑ®g@©h­¾i³@ªÚÀ«VZ¿ãH4qC0¤¿èðݯte¿ä=`
¬¬¿çõȝNk.UNASNone?zA_Ýé?€+]ñR×u?‰Ë;`ís¬?"é6$MAl?ïdPRÂ=ö?—ûld)²W?ŸŸÖ\&°Ë?°ÏðNQK?©GýøÎß?­Èm&OäÅ?ínm'܈?¹
‹¦œÜ@?¼\g'&rö?¥²p¾?6Ï?Â<šˆÙ¼?ªµ"Åh…?çåL…øû1?²ä·*a±?ͅÈ5Mq?Á5mòŸ?‡µ/ˆß?'"V'­"g?è?äY4‰'?Á'ð}1ðî3FGL J1312.3+8513@^šâ:¸c@?á鞔«À:5-ø`ÏNÀ;ޓ*êU?Ó-}*'èº@
ì¯úÙû_@Œrk­¿èRÔÚs«¿æPÒLàѿ旤ØÿпÑÚÍì\ŠUNASNone?ïߧr¥¨?váÎC€?aûÈ'k%?kKûjk?]äwŠeÚ
?l[àäÌÜ©?îïMڲË?©ïm¢HÛC?"™‡µwáz?¡Y"Éé?Œùyè_Z
?›;\SyÏ?î=….;ùc?"݃üÉ?'´lÂÔÈ?"g6½è¢?¢Ív»1Y?ÄnB^ê?싙0ç´?¯N0cÊçr?£[®¾ªU?§'6Ûyé?±õ_m4è?¥þ²ÔÕ83FGL J1315.7-0732@s—+Iº@Ki¡lçŠÀ9f'áÇ/ÕÀ;'N+Üýœ¿ú0qÅ?9Ò@"étù&@'JßÍ/ž¿Ìß³={¿ß,Lâx8¿åœVK·u¿Æ·ŽgUNASNone?ïøü#R¦?G¶F?="юĘ°?=‡>¬°?>]MV¦6Ï?<ÜKÁك:?ï׉Ix
?w…¿ªýZ³?bÔá"}±­?mŽ—á8?e¡Õd
C0?l'Þs|Ú?îþp]^}T?L
6ŽÐl?lûâx?‡£dŽ_!?1cç4s?'Wæ›B°š?ïâ£Î·Å'?l#i_ˆ3>ö&>`>C?	L˜[Çì?m0
û¾§?kú¨?é3FGL J1316.2-6446@s/D')‰À3¼$ÞܚÀ8{¾öJt˜À:Åe˜Tö?à;'1ÈúÛ@¨/t··è@O"/û›¿èeà
éš¿èd€k'ôÄ¿ìÈ`´u½ò¿áÝüó¹©7UNASNone?ï^GkJÕ2?—á{"Ê$`?qþÌ^»\?‹¿È*úae?†ü&`ëøA?~O÷¾Ä?ã^(Ô?Ó^•&Õ'D?©U<ÉR?²ZÈÅ4!?Ö¬™ZA.?ÑüCFõ›è?è6n:£Wn?´64{Ǻ?³¤Î÷­Õ?£zWXÐCü?ÅT>-öË`?°-úDüÒ?ë41ªƒXb?­»sM'‡|?€Æüjïe?v–=-?Â.Ìæ+ï?­f"f£µ˜3FGL J1323.2-3901@sZ‡ÝDU@7nhãï(AÀ9ËøÁG^À;q½OH¿ÙõÜûîùG@ŒÖ脎@.Yßð@¿ãÍZÐc–¿èœ±ûÔææ¿ã`C˜õɊ¿éh=2v±UNASNone?íi[ž7?µ.ú÷ÿÊs?Gth?'Žd	¹Ô›?³[Ãyü\?³²›­?îøH½'	?µ†Tþí?'¸Ä»2G?iÎW¹L?Í|G?Ù'?"ëûžf&†?ì¬Ü.k¯Š?¢ëÌGˆ?Ÿ¾bÛ7'×?‹fc‡=P?²©…ÕÔ¹·?žCûÒ³Í?ê"2Å$Ò?¨ÀžúÙÉ?"¡ÁÚYmƒ?‡q"=€D´?Ã>ü°!ŠL?§»_$‹!3FGL J1325.2-5411@s>¼¾aÏÿ@ ·;dZ¬À9AŒa¢²GÀ; èN2'ú?íñ—Ú;w@¥®¯*z}@Ì€•'¢¿Óÿúܪb¿ä=,°sa¿éX ÌSU¿ïÿÙ14*UNASNone?ՆJިɜ?È·Tœßž?ád­¼žŽÓ?Ì9ˆÃ0Õ?¾Áf hbþ?¿EYGé™?¤úµŒ(â)?¯SǤËz?åb¢4ç‡?Èç4Yó|€?қe8®?È*5f8b;?Üóæ¼È??³ä4{͑@?ÕlyÓ(s?±äÿ|×È?Ë@áòàš?­CVß:l?°˜·`T§?žxUéÞé?ç¬235Ê?ºg÷¨Ì$Ã?Éۃ'?µÖª§áÐ3FGL J1326.2-4651@sQÀ­Ú@/4ƒì‰*·À9ÕÜ@WÀ;0¥:·‹ó¿øÇ6þCè7@
²¨óSÊ-@Ž— <A?ïíȬýj¿ê¿«aB:7¿ïþÍë'MC?ïó
ƒ½²UNASNone?ïyËláýX?¢÷ÞÿX?rÔµpÐF?€É`®M?ˆ#lÈB?¡ûèŒkÍ?ï9*Ðma?«n±'"ôï?ië‡ýw¹?…4C,øÙ?•4ò®Üº?©¥my?é£q@8[?¯ÐDdΚk?¬Þ¦5gÚÇ?™šG2_ï?Â:'qŏâ?¬gâL@ºv?ï‰9iMjð?£íˆáä+>ø'NU…b?÷Ñ´¨–¶?¥¥k~#?£	;°¿¬3FGL J1329.1-0536@sþà"'@LÆ)ñkÀ9ƹ#¢œxÀ;@2芘u¿Õ?Aì@esˆ¸Ë¹@Ð
€CR¿à'Z$—¿ã°q7!C¿ààAƒOw¯¿çt¯œ\¹âUNASNone?ïƒB0¢»?Ÿ­üã«:?i¿ìàäÍS?j®;M](?ˆ¿xŸ
a?Š®_ƒp?︈¾gê?¯'
˜?qé¾gèsž?v®8®	?qÒ?8ã—?sØæ'œ~?îHKä¡?•8Í&ûÝ7?'é'MzA_?'¯Î^³Ëa?¢†y2/R?þÙkï?îDž¹ì€?›µKg?oFPöâÂò?fž«]«¿ ?­ÇQóØ?›1ÓTò)3FGL J1330.4+5641@\
gbé@MТ ©XSÀ:dš,fXÀ;øwéE©¿¨Q&#°RQ@OƒNÿl‡@öê?yg ¿å,öŽÖâ¿î–56¿¿±^:íU/¿ä!q)búÌUNASNone?ï÷ƒf·"?e£ž½k_<?#öÏ^nF?`‰±¤"g¶?Lô±J,ôã?Y²PðÔÈ?ï¸9uX9\?†qτ®r5?qç2s­?{¼:/AT¹?qü/!o¤?yIkšr?îí9{&Y?b*h Ý?}?Ž÷ÒN?ušàˆ—=½?›ìÝpŽ? Ghå ?ßG
n?Šà"ªËŠ?Eûâ9ª?R·'~JÀ?‡6ËôÉü?‰lÉ]Q
3FGL J1333.8-4417@sn#9Àëî@1í…zþ£ßÀ9žs;`ÿÀ;R`ÊE3¿úœ¤cL*¦@ðwÆO@}þÿú̏¿èj!Ù­l¿ìFÂer ¿Â¹­åoÊ­¿ëÝg:UNASNone?ïáŠ`?r²Ž"F?Tl¼Ú¸no?]ÍÉ8¿?d?œtžhœ?m TŸá?áýÙh?šÅð"®?i~A)Û¡U?o±Uý®'[?†ø76½ƒ?™( Œ)/W?ì‹5
K'Q?¤à‹EŒZñ?¥—"z–S?"<ÀFÌQÉ?±$ëf¢N?Ÿ+œïqI4?î Ãmø? }R`?%̀ÿH'ÿ?9äÂѳ°C?¥Þ^	ØV? vnPÖe3FGL J1334.3-4152@svçl‹C–@4K=áâއÀ:–ßY—KÀ;ºXVk¿ªmyÝ@
4yeqžÔ@

ŸzÚ¿ÃB¿­ªr°¿ïþ¯€ê(Ü?ïè÷·uçR¿ãîüúD³UNASNone?ïÎvp@U?Ž¹Y[µ§Ê?Dá_d¼°[?YsÍv]‰A?v(›ó!¿P?Œ¸bÝöC?ï¥Àݞ®¢?'읜Ï?n(([ú:¢?zÓªùðÎ*?~}«'ó?©›
Ð?îœBᘤ? x%éb?‰"û;Çg??zàg¬q3¡?Ÿ­¿%é7Ó?…Hb?WÙ9?±7¹ÈK…®?'·Hܐ-³?Oµ¬Šä0å?§}S9ß?±6;iƁ†3FGL J1335.1-5655@sNSŽóMj@Ã֞ݦ9À9ŠÙã5ÅÀ:þIc `É?á¿0rþ>@Å0Pª½X@´8àœ7"¿ßî·§»_+¿åÚä_ð¿ÝQùX,M¿íö‹ÅùýeUNASNone?çY*͵¾t?ŀ<¼ç€?¡M@à+Y€?ŸÅ&N™:&?ÎH'/Ó?Å
t`[(?èCÅn|AÔ?ďåê"NZ?§Ò+ç["?›g9=(Ô?Ë;ð'
>?ÃP¶Sgx?åðÿ}2Þ¼?¶o'l³n?¹£,eE˜Ü?¢ælϑr?Ëjkؑ¸Ÿ?´²¥ÀÕ?ç}׆vvp?°Žy$ÆÃ?¯
Å©?"$|L¦g?ÎeÍq?°èý‡'3FGL J1335.2-4056@s|quŽ@5.©÷µ®£À9R%cf×¥À;Ov©ªˆÕ?ÉAy"÷@]EÀÔq@p[­Š<¿çÙ|Oa¿é㼊àCL¿å艧ÝÞ¿ÛnÝzUNASNone?ïÀ:G™ã?€*è¢Í&?f‹ÖSÕÇò?fQ0aú=®?tœñ	#˜j?{18ã?M¿š9?"XŠ(à1š?{¹"ZÚðÖ?"É`??t"b«ùX?‹ˆ-i'¹?íêÊz)±®?œñöcG·ø?"äÁžj`?…n×PŸ>'?§`÷Ž/–o?—Hò˜æ?ìæcž9«?¤o¢`)pG?ëX‡?€§càê<º?¹^wü²?¤(ý3,I3FGL J1342.4-6904@s7ÃAž0À›s¢¡À9§vÖöò:À; ãœòên¿ìÃ4ø@È-*Ûv@8¬Ë¿æöfÏþõ¿êô³|>¿ÚËàiÈ×±¿çج˜5&ºUNASNone?ît°JRN"?¯Ç¶¿ªà?`5*Œ7Ž?eÎ/
ö…Ž?§´x2S8?¯'{X«•k?êäégÞ?ŒCS;?"èó×̉ã?Ÿ¦º¾™Yô?ÁÒÉI`ÏL?Â+µá]é=?ë>ʑ{jm?ªÄutgr#? ç9Bæ±?Ìv¬‰Å&?½ü7׃9E?§¡vç?éåõª7=Ç?µõºH|Q¹?\O0ü¡"?[Kto~C?È/Šõ)ç¤?µôýÕåJ3FGL J1345.1+1949@}Èû†ô{@RìÉ.À:?|èˆêöÀ;Ïòü~¹¿Ø†
á/…@mìðƒ¶@Ò.@Z80¿é…U;¿æa3æÙµ¶¿à¨'v'È¿åìb?vs¶UNASNone?ïÛô¯ö´ª?'Î͸^&j?:H@ˆF?<'ÂPžª?pa#ü!Iþ?'`bÊŵ@?'[5?Žu^WìtÈ?s<—ÿèÊn?|ÏW@:¢;?|ÿ&ҕ´?ˆ'º
°ÿN?î¸ÛóÑ@t?"'øÖ{ÂL?…}<·7?w+®b~l¹?žøG9•Ø?¸£êÀ~?ïNTûû"ô?ˆ™Y>Yõ*?k±÷¾Uó…?d´¦-ª?'¿!ˆÐã%?‡7/úÜ¿¡3FGL J1346.2-2608@sà)~+V@A'Ó"vóÀ9êwXüñXÀ;³$™<|ˆ?è6'Ú!@‹£š#';@›'`—¿ä•ë8âí¿âÖ^¯§è¿ãR]ƒG¿ìÂ,G(*
UNASNone?ãúÔìûì'?őqYF%8?дAë…?Â_ÿ\?½XTHt8¯?¹³w!´&.?é
%Ê1Ãd?½V:«3?ŋ¢(|ëâ?¹™³M±í?©/ºð??¦[ì'ý?êt›O8¯?¯v!¤EB?¹LLq—j?¤Ëƒzµºj?³Ù£T? ¦Ø¢$&á?å^ƒxïsb?³RY®#Ô?ÌàYÕÚ²?²+6¾ñ"™?»K±"د"?¤ÇIJL$g3FGL J1348.5-7150@s6t¼j~úÀ"î%¦'¶(À9¼ÚH¶RÀ;ZÐW›È?ÚÉN[5cm@@&=+""@€¥+ô¿èWt4¿êÉiñ5aâ¿Îž.bج¿æêÜØ2±ƒUNASNone?ïÙuY[U?€Ë_'(?4"_"é…?6©´2ðÉ?r8Z?¤Úvñý?ë…N*¦
Õ?ÄÏ?'uÓ¸ù?—Ì5¬>i?¿"ñ6	£?Â"å't»?îM\¹2à?–ȳ4Ol'?ŠPü£ý@G?™' ?¤•õCÒ§ö?"
õDÞ6Í?퉁%¨ñI?¥ÿù]{Øh?bÂ}²×Ñ?gù'¤º?³æÆÊÞú?¥¹³ǔ%3FGL J1348.5-5833@sezÁҝÇ@ß°&£Ø¸À8ô´JÀ:æ$óÅ?´¾ÛÚ.@âøc!@XKŸ©†¿êL:­>ÖÄ¿êYãñ#ǿ׆£˜ÞÖ¿ê¤{X™}UNASNone	?é…-`Ыþ?Ä­
¢¸ƒØ?ŒNjmRH?‹6ƒfÌ?È)^zç?ÄGK#g?èŽCF'h˜?ȌËn²pA?ž
³3
Ù? ŠP‰ä1?ÊœYo?Æ¥½ç¼©?áFÌ(–&œ?ºÚLèS?º†\¹iù…?¢CŠ×œQ?ÖÐЀy4f?¹Ø `Ú¨?äuߎI2v?¾eâüÊÍ?b¹¨&´?‡2æs¿¯½?Ö+]Í Yß?¾uØ֜F
3FGL J1351.1-2743@sì^_0çÿ@@§T!ÀD(À:¿¦¥òÀ;šCV–势öÀ)æ®JV@!¯B"dY@c cbP¿ÞI]褪ֿì?ž8dË\¿äóC¶……¿¹~"d%EUNASNone?ïèÆz0KÄ?gäiÈGˆ?A(×ôšò¦?AÙðF' ?bïOҍ×?f"{m#OÖ?ïЊTvF?xjÛ4A?bÿ|ß '?g0ý—k[p?lv
™y?q뤛B ³?Îð$Œ?ù÷O1€?‰"ò´÷é?ÿW'qšþ?›lŒÇì"?‰Þ­T ?ïÇÞw"îN?tã­ÿ9½>ó³^Ðh÷Z?½âúâh?{ýÞ¸pL?t߇V'3FGL J1351.8-1524@t;Ýcˆe•@FZ³R¨À:E{°z†¯À;•
ùXF¿ËùÈä
4@Ğ×F"y@4`JmŒ¿ì¬ €Ò[¿ãçäeI¿â`ÇúfIF¿ÕùÅÈexÄUNASNone?ïöµ£v.P?a¥'Hó×?=<VÁêZí?@6·ihz?F‹FÆQ'Ó?]i
,·¿(?ïÁävW6?	÷å«G?o²É¨vSš?x¨Æw%Ñ?nh¿Ç2u¾?qT§d[ה?ï$ʵF"Ý?‡'Æeþ5—?þ™å‰k?uà-Ëìò?'g\dj®Û?—¥8å
1?ï…{ÉÓUÛ?ulõ¶:?BLb0f
1?FRþ'‡óþ?|Gh$(‹?€ÓœèUs3FGL J1400.2-2413@t&©Ür\>@BÖ¡aä÷À9ÞvlmçdÀ;¤ñ-À?ó¨›C@U;ÉÇ_@@Óàx"¿åÞ÷*T£'¿Ñ²Å1u¿äÈò¯3<¿ïÿúÐÚè2UNASNone?ڙÊhûq7?Ñ1©MÛ{?áb@¥Aj?ÑR…q8Iæ?¥X­Ð_'?°>^0ì)ß?ÑoõŽ*;?Äw#üT?äýë,l%?Åýïj홨?²RnÆf.3?¯©ýµ
âñ?؟År7[P?¸8¹"èý?ßeˊÊw?¹I™ï:º?¿é¼ø¶¢?¦Ê´!<.?Ó`÷}øL?·¡¡Ñ?ä[xÁ{dâ?ºìÄ×åˆÄ?¯@·ø‰—‡?Ÿõc³3FGL J1402.7-3240@sþ=ÈK@;ØÃÁ‹P+À:-bŒ½EÀ;´ê8v¿×wò.J@Ìdȵ@‹\@r¶×¿å*±Pg¿ç`ƒ<ØE¿é7ÞS¿âçƒ(áUNASNone?ï¹T€Þ?ƒ¡Âà*?au}¹Ö<á?cv_}7ül?z›rT? &âèZ?ï¥Xgm?‡,«·'Ë?tfݼvª?xûÂvº*?xìîŒþìÃ?~VU*¶?{v–?'ɪéfâß?n‰"¨"?'ÊJr¨ ¾?œ4Y‰GY?ˆ2]írï,?îéÝ
"'?'vZ'®3'?i‹.R»¶?hf:¸6&ñ?Ÿ'øÓõøù?'ów%Za3FGL J1403.1+1304@vH'ýuâ@Q—á2µ_À:Ájî‹À;ïQ{×?éüQ·Øžè@ÄîÕÒ°@ +ßVè¿äÏì‡cr¿Û4¸#G'Ë¿è|&x¿ïÿ"¢[VŠUNASNone?êg3òiÔ{?ÂI*‹Ñ'â?Å1_?s¨?Ââ²bï?…ïíq"¦ÿ?ŒæÒrŠJ?è¹|b;\ˆ?Æ7Ž'ɐ?ÆÔlT+?Ä$^Ýí(?©ˆ‹Í‹8?ªSÓq¬:?èk`}č?³ˆÀ~±§I?Æˊãˆ0&?±À¤ºjw?®̕–oJ?˜6	õþž?à†CåÙ?ÀjÇ?+_Ù?܄6]"gN?Á‹òPf?£|ˆãh?™ä`3JHí3FGL J1404.3-5241@sŸ¬1&é@!4úïõÆÁÀ9²ä¥5¯À;I¼2JÕç?ê­-°Åã­@ޒr@Щ¾€¿é½«û#«¿ÔÍ6ŸNdg¿ì/¤`p¿åL²Æˆ²UNASNone?ëy_v¢"?À—Ñ!¥¥Å?¿áÎÑñD?½µ=¿ c?"¼‰ðfH–?­Äó*1^Ï?ìG>ôÆ?½Fè_(£E?˜&0=­Ï?ž>[ØÒÿ?¸üE¼Jcž?¹gïý ðW?ìŠEètÆ-?£z™Ä
V?ªˆEÁ€Àþ?˜••£Â<?¬Ó[·2Ü'?˜­+Ç̧Ï?èzXEœ9?¶£þÅBB?½]ýPZ	?´$ê³<Ej?¾Ò2@'Ä)?«
Ã"''43FGL J1404.7-5844@s…d2‹n@Ki~J‰À9ªÂ©][üÀ:ÍçâÒÉ?І5lQ@
Y»~Ư|@U]ŸÃTS?ï=p?qô©¿ìñ£êƒ¿ãv˜@[ÿ¹Þ'$¸ÏUNASNone?ÓTy?¹Ñ‰?Ïü°Nì²?q¿~'šu?y4ïÛMŸ0?æ2Dc?ÐišcOh?äkˆaÝ&…?Ô
LøRE?"sv!Mc?¡õFݸ¼?Õá·Ûãž?ÓKï·Íëí?à*Œa³šÞ?¾î®•#Ž?±Û'CD¸?¢™Ê!ú»?Û4«ÇÆV?¿å÷ÂA–?åã
s"ƒ?Â&H¥mî*?gýHc:Â?sÅëó1?Ô	ùTRcu? ¢¾;‰3FGL J1408.0-2924@t%܇Tó@>'Z³R¨À9®`À48À;±£|qk?ó13ú-ƒ@pù½EÆ@|¾`xe¿äÂÛ­÷ZÑ¿ê(߀6NÏ¿ìû+–¿í»ÓáûvUNASNone?߂Ɩ9[?É?oÏ/Ž?Մ6žÇ?ÈÏ{¥ãúø?Åò¤µƒ¼?À¾x†R,?ÖæèV… p?Íå6Ž3"?â:Œé6â?ÍkHëå;Ž?²÷\4iÃ?±:ªY‰Y|?ãº1—‹±1?³š¥Ì3>?ÑÆWƒ§?±r—´wÖ?½ÓYå–â?£9Õ¥Ç?Æt"¼ú'ä?²ÍÃ1f?çžÄM"‰9?»ÜQsµö?¶!˜ö°j?¬!…%Æ3FGL J1409.2-3743@sø!-w1@6¢DAxpTÀ9ÂÏL
ÑÀ;•e×y¿ïݦXނ@1›Â"¸Ú@—Iÿ¨lE¿ç<Õã™9o¿ä•ìÐj^¿èPâèÂø¿ïÿ‡{£©,UNASNone?ï®·["K?Ÿ{ }g?Œnæ‡)"¹?'Õ3†Q-?‹åk¡õh?"	²"îÈÜ?îóÏôDƒ? óN"ؕ?'|rM½†}?'–˜+å?	ª3¹é*?•iÆJ–ö?ì.@é":¢?¤¿óÛoÞ!?®:ƒ_ú?™=˜€&Î?®ánªPÛ?š5{¢Ü1?ìéû~-ð?«gZb¡Ù?˜ÈÞÜÅ? 2¡^7Æ?²}ðÝJ<?¤ìûIÊ#3FGL J1410.9+7406@\ﰉ 'R@DòF¿2/À9›ÖøjÀ;ûœGÉÃ-?ñ(ÆGÍt@.rÆÆù@Q_Vý"¿é÷£Öâ¿âEu³"ô¿Ô?Èå.þ¿àOœ&€ŒUNASNone?î>{[Òa?­G)ÚC†?¢©«˜ð?§"›!¾X?"A.ý;?˜q"ñ˜vµ?ì6B5á"?¾-"ˆxì?¶^ږlÚ?¹ÏÞBZÿÌ? ìÂ?¤KYuºl?ëî瘙‰?ªC"}Æ?´CE^z¶?¡±är(}?²õCdÀ}²?Ÿê7ðêÇì?ëïZtʂÛ?´à'ï:µ?²9I go?±r—5'€½?¬—Ær‰•{?¥ˆÁºdÌ3FGL J1411.1+3717@QFȟ@¢‡@Q—hƒöèÀ:nêžnëpÀ;ü jÓ?ÙÛ3tì!@
¾¤B¿î@ÒäŸý5ö¿évâ0Ðò¿è×Ýú#k¿åÈ-§iL0¿ÉÛ9B†UNASNone?ïÎ[£f?Ž¿¢<Å8?fIƒ"VÊ¢?‰7"Ö§ŒÏ?k[vÆÏ ?/Õ=ñqe?爵­(x]?ŽJ6¸¤Tc?tL2ÕAÆ?ƒØýŒ<?vdv–¾h?'mRx­?îelKç!?"!ü>_ß?'w[ ?ƒ¸¶Å‡
?¡¯?…à#?ŒX*[ÆQ7?ïQ2½wk\?'€áwRõ?wâ¥'?¸^¶mäý?êߛÒ_Ë?Žªg®4p3FGL J1411.4-0724@tñ ä¶1@I3]9—À:†ÖHv'À;³c"GÁ¿æ¶twºæ_@ñGÊDj?þ]Û O@Z?¬U#I»?ᚌF'Š;¿â¢át';¿Ñ-•ÇIwUNASNone?ïÆÿ¿2^ˆ?Ž«…ôñA?U¸Kz?YDt«Hê?wx½ôs?¥¨n']¤?︥d±É?†÷laîh ?tlÙÔW?'•ßA'Xv?oրçǘ?u¶ÐÕA'N?îµð]¬–?ç~Vâ½H?"!…׿:?†ÃN˜Ld?– nr®ê?'ä솷?ªJ£\?…žC†""?p¯& 5?sëâò^	?"¼NlÃØ¢?'ôùy\ó3FGL J1417.5-4402@síÒܱF_@0&s>»ýrÀ9W€•ÓÀ;h"¡T¢?ؕ0›JÁ@&"~…@óQŸÚÑG¿ä'DˆÆ¿¿ãò[/Y=¿â{Ë¡dÐJ¿îØv°zJŽUNASNone?äÒK¶ŸB?Æ[úØ5›>?ÎÓs(4f5?Â?³?mÑK?»Æ»úž¹…?¼(	$ÔX~?é/¡[™ð
?ÁCÓ·va?ÀÑÐUmӍ?·asYÜ7?´ßTxT؃?´Y°ö=?旴€jân?´¡'œÈô?ÉÌÌþ²ª?± Á#:î\?¹*Âb«‡B?¡A×â_?æ½ùÖP¯?²ò5
ÓüÛ?À÷¯8KZ?°¡4¾ÐÔ'?Ä÷ ÷‡Mé?ªN1³—z3FGL J1417.7-5026@sËË)^ž@$9¹×ý'wÀ9u΁eÆÀ;7E¶Ãv¿í‡‰½AZ@
­^܄OÛ@âZߟO¿ë!ǕLÐ5¿áuV^¹ýE¿çMe—¿á÷¤DîGUNASNone?ê¦}ñ¸¤?ÂÃÐh±ø­?°Í#û?°'6|ø^?º`'v«Í?ÀnÃå .?íðP›úö?´9Oíò™?€»^«?ŠB+0•`6?¬Ì0¨¾Uç?²NlÒܧ3?êôåm'Q"?©']¯¯f@?¨¨n˜˜ò?"K­8?¼Jº*u?¥=>Äé?»?ì»$'
Ë'?¦u
œ<?lm˜*ý ?nÀåF]?¹CròÐNã?¦3û5'Ö3FGL J1419.1-5534@s²³œ¾à@Ê'ÿÀ8Úoõ—ÇÀ;õ€J=;¿éݬý4Û@ÏJ€Æ@‡·ßªÊï¿ê˜úpQªJ¿ê~­øvHÝ¿ãèw¿êÛqÒò´UNASNone	?î$¥ž9¥Ï?±¸XA¿<?x¤ÂT>¸?|?ΧÍú?ª¡
ÑÝà²?°©»¯®?ëlw*÷Ž?Á^—'Óòb?ˆ='gÀ\?ml"‹Å?ÀÊJ1h!?ÀdâŽ&V?æŽ'šI@Ç?µÀzŸá1¦?¸‹j&b¶e?¡ïՓ%¾?Ɂ¬ƒ©¡°?±£^2ŠG?ëKÃú¢G½?­ŸÛ(V¥z?o7;RoRj?pè1¡›Ê?ÂT(-#Á?­yêKÏã3FGL J1420.9-4615@sê±[W>«@+¹ò™0À9'Ùe5À;i@։äñ?Ð'ÝßÄ¡/@
Á¬œU¶–@›¥^¿ÿ¿ë"¶å@a¿æñQïê¿ä3½6¬º^¿êÌádßR¶UNASNone?ìuB¼r>«?º+e
Ì°?§ª6‹ôo?«a‹5h?°€Ï¨o?±ñ_åq‡Ý?ìú˜s?ºf‰I?¨¨ãÍ5w?£DRKü?³CãM…Í?´Ü`_~Ì=?ëê^\Ñ?§Üe&Y¼?­1ZµRH?–MLö''?¸wÿ´\Ñ?¡šêUe›6?çql–É€V?¬Ô«4(Lš?´=Š0k…­?žhÔA±ÀP?ȈŒ¤;Î?ªsÌÊô€Œ3FGL J1421.0-2431@tzzcslß@A¿"ÀiÀ:…îÁêÀ;²';ýP?ìPó/›@Mk›Y:@šÂ?U*?àZ¶_ևê¿áü»yµšù¿åÀ/@Æè¿ïÿ÷,OqáUNASNone?çE"&†?Îì{.3—Ó?Í'ƒ
X?̉÷%f"?£OgÑo}f?³Pçݘ£?Þ»*þV>?É&8΅
?ݒ‡i"?7?Èqƒl-¨'?±fõ­õª'?¯G­…²c)?äm¥Í®'ò?´Žù±B)Å?ÎZú¤?±á&RZ'4?¿Þ¥Bfm?¨â튈Mn?×8ÁÃwö?»Àí«¢l?áAâ2¸Â?¿°ôK¼?ºzéàö!?­|SÛtŸ3FGL J1421.8-7920@s3.œË}AÀ1;'`4PÀ:0«ÆÂǐÀ;¨Ò3>î?ð™@Ù9Í@0Ç˱ç@&@tdV?î àç?¿äªÔÚ.×{¿å½'T«ÓÙ¿ê«';…UNASNone?çÞòy²Sy?Å	§HÖ3½?À_‡1ìó?¼cûNµ¨v?À%'Å(?º¾÷'F?éØà;'‰,?ÄèÞËïD²?¸§ 
×d?·ÅºÅ†êì?¹,Vƒ]ß<?¹Õ«eÐíÉ?å/1tܔí?·µ>†>2?˃7¬·?³H2Ž÷™?À)¶ôàô¿?¥GʸÈ&?áÏõGãD?¼ø;fcó9?ÎYŸxE;ˆ?¸lL÷¿¨Ð?ÊfŒz›7e?·@›í)¦]3FGL J1424.3-1753@tÁëíúCþ@CԍûÖ¥"À9äZ#bØÀ;¤Wë‰P¿Ún,£¢%@1s0Ï*Ë@c]a#Ü¿é\~éjl¿ß'"®iÏ¿ÞÆÁk«ÛÍ¿á§ù´"û-UNASNone?ïßË<àb?tþè°t?MMR'd~ž?JþÜKÁÿ?hán{X~b?s&û\;4?ïµÚèè¾?€_¶¸-Ó?qkVú`T?q)ë+°¦›?tw'4'@}?x›҉Ζ?ï4›Ý€y?ˆüd¶??JL¡Gù?u"Ê{ó€D?Ç]ÿHÌÍ?ƒ<ðØ ?ï\«žRå3?ƒãOä«ã?Rºn
nw?Pú§w£!?">åKÒ²²?ƒuµ;;;3FGL J1427.2+1610@'.'O"}@PPe¾ ºÀ:¤.™À;ÅÏASCÀ•Öé±4@;cÃÉÃÙ@O?ƒM¨¿ê/¨+º÷¿èƒžNEn…¿æ‡iJ"Äe¿ïÿqñp+rUNASNone?ïõƒ—'?Xöà"MbH?<½ýÔR`??ûóI£¯?K_"¤yªü?TéQrt¶?ïºwõ]ûã?…;'Z¢?n^k>ˆïy?wñ¨4›J?s"ϱ½–Á?{®]ÏÎ
?îbÿ¾Ñ·'?•É;¹;#?—vOÂ#Ï?‡OùhvL6?œŠ'Öëì?ì+kÁ?ïkÅ?~¾?ŠØ¡µ;?Wûv¶Mi'?nÿ¥»àŽ?‰%ŸÙV£t?ˆwy£$O3FGL J1430.8-4434@t'œàu÷@-•Ã½Y'CÀ9"Ü%/drÀ;nú|2€†ÀknY$	@ø¼—u}@Í?†'Í¿ß×ólàf¿çIš†\.¿ÝvÑӜʧ¿êYIä5Û?UNASNone?í~¾q'F?·ÞXœÇCL?…]`ó&n?"IZ¾å½4?±^^ö©?¶áUùtè?ï7dѸ}?©ÞŠÉÜç§?hvÀ×lgº?rŽàÂBB¨?™J;JÛc…?¨³܎Øk?ìt4ž¬¼Õ?¦pCªÔà?¥ù"s™8Ñ?"Ç"‰?±aÐÍ|ô? èÕ¬Kø?ï\XDÅ?"OÌ®¨Ãl?b«n¦'?2׳ÿv|?"eMiÚø¿?"D=Ü"í3FGL J1431.1-6425@s—¾ß¤@À؅Ó7ëÀ9K¼šO¡ÿÀ:þ¹™aÝ?æú¬ä•T@›5sñ@»Ÿú[Ñ¿æWþŽ]GÑ¿ê|˔WT?¿ãÀ+Ê^3¿ïÿÜ¡"œZUNASNone?îI7€© Ó?®á~És?feeoÚt
?ng'Ù¾:?ª1žpKŠ?®ÐtÄT?Õèäï.?ÐîPñrb?À¢X';?¹Ù$èé?àâ÷ï'Ä#?κ»S9Xò?è'Ípä?¶êãg0?­ª…ԝ/?šfµ—žd?ÈSVbÕ%?³àÄ´µXd?äWÀøm£û?·4U|/ð?¬hªˆ°éÈ? ·Â°$d?ÓÃh¾šÑ?µÏhg|HP3FGL J1438.6-4209@t5K}At?@0lˆçš®mÀ:
xë¤(iÀ;fûéðÊ?ä	©`¥Ì@+-Ïqï@'¸`.>¿ílŸæe¿ä½4ºƒ¿ÙSÞ%²
¦¿Ò¨"^F\[UNASNone?ï·e0ñ6?¡`6¦
Â?tBµMÅ"? "ÖûžÆp?p
"öŸ·?"s¤ÎõDÁ?ïE›ÄÓô? JÖDàÀ?€·…Sv"Þ?‡b©_²åÈ?á‰wÄ~=?™Û¤@"oY?íäTл	ã?š¦Ud…6Û?•¿à|
ðb?†UFRó!­?¦Ú¶Hi'?•[•–æS?ëÛ¡QA?®Õ­"&¶î?ŠÐ¸`-ñ0?"øiÖ`ª_?½ÈàO·Õ?­"á.À#3FGL J1444.0-7033@s'ÂzcsÀ#r-"ÁÀ9æÆ:"‰À;™jZÀ†<¶¿š4@
u_þmY@–­ _¿æU¶ëè=¿éDT@(4¿Õ$8܌ֿê-h(»éƒUNASNone?í,ç0dôo?¶îÍvƒÁ5?t_×Nã´w?xQ]+ ?µRÉê!D?¶~®‡Ös²?ï)ÀXf½Ð?¤\Éf"ìî?k[KÈä÷Ó?'©u ¾Òˆ?—\‹z¦ú?¡í̘¤õ?ì(FÁMš¨?¥Õ0÷×`?¢¦m`âÝ?¼I!+ìé?µj"E‹¹Q?¡§3ÿôà?ï?ðõæÅ)?—3#*s>p?hø!BÅ?ÊIâ'E?—ù,Ç͟?—-záКD3FGL J1445.7-5925@sÐKÛ ¥'?ÑèxD4b]À8¼~Ù$À: ^ØP?ґ£¥zè@
~p+—@»;\_¿ƒ‡éÕY€Õ¿è%D
y‰6¿éW"#žô*¿åc}äd÷"UNASNone?j,½`?pül[A,?´ü7DäIº?½9¨È?íFmêÒ¹h?½aU°´¾"?Ÿ5m]J¨?¬ðé…Â?ªà?6G‹?°6¤ëœ£?íXP¦	±2?·¦¶u™7V?Â\L'ðuw?¨1]j¬2o?ŖÝS䌘?¯iÄTæ*?æ5†J¿}?´-!,™H?ý]ƒ?¼³%~¿"?›ä!¥Ãr?"ì›I$U?ê`pMÛq#?¾VûÒÅä3FGL J1457.6-6249@sÌn—OßÀ2ô™špYÀ9;ÛmiÀ:Ú
>¬ãù?ì^bq`@žžô@™G€r+A?ïË&´A2¿äI
¾À«½¿íñÛØŠõ¿àÆ\_SUNASNone?Óq"ü«û…?Í%4v'Y³?ݖÓ)•ßŒ?ÐKƒÔÁ,?Íï/³|IÜ?Ë0\>Š,®?Ï¡uÔ¦?ÐZ	>á'†?Í÷¢8g+'?Èð>\ƒp?à™ÐTqœ?Ïk­ÉïØ?Ý-ÅÙʸŠ?¶¤éљp?Ç^x³¥I?±¤Æ$¹n(?×"ýÌb¢ç?¶u'£Ú?Âgˆ‡‹‰?¶ZŸš¬a?Öý#'áý?ͼMr#Kˆ?ßô¨©Ú=8?ÊcJxvP3FGL J1457.6-5355@t÷zö@d@æK©K¾DÀ9™'W«¸€À;	……`ý?ÛIÝޘ¸@
1$¢e@Y^ðá)¿ç|m(CãQ¿ëݞc­Ï\¿Üb–#S¨Z¿á灇»0ÿUNASNone?æAp©p_ø?ÎlïÆs~?€ž¡ÉÜá?‡ù"ÂÈÍy?Òø)žÐ_²?ÍÐNÎlS?ㄸ®­k?Òý{Ée'=?š©Cži?¡'íìY?×Ký¾kBe?ÒEÕØ÷Ép?覗Úó ¦?³–ÝP¼	Ç?©É"¿ÈÊ?›gR1Íò?Ç%nKƒ‹7?±n};¼I?çÇ2¯Šˆ?º²4¨§?ƒmw4É?…Ûoô—2?Ñ9¢-1H?¹¶Ä–[33FGL J1458.7-2120@u)u\)@@JŸ±À9­—1àLÜÀ;•ÈFUNç?âƒJEžp@†úc
@»Å@;"e¿äËOT"š7¿à®îaᶿåí?}̒¿ïÿ°yÚâdUNASNone?å¡á÷œ}?ÈÁ7D@%?Ñï%Ø`÷?ÇmZnÒ?¦i'_£0?¥‡òÒ92G?Ó£|Ûµ'*?Ç¡Þⶹ,?ãËëýÄ`?Çø²Hºæ»?³¬£b©?°{a™8^"?èj‹‰Bî‰?°¤e#œ'?Ã,Ú"Y»¶?«§Á/¹¿Y?¶Qïq5C?Ÿ'!ƒ>ª?Ô-'›BL?¹€ŽN›?áÜvÕ¤:'?ÀÁ€X¥r?À3rë"?­{?[ûB3FGL J1502.2+5553@W2>BZîc@Js,­'À9},²æqºÀ;îW"KS»À	úf9oã=@‡Þ@ª£ +²¿å9_¨Þí¿èëBó^uÆ¿áÎÒǞ̿ìOq4ÿUNASNone?ïøÀi'ö?Qëx߬c?'ï:
N?1'"òLØ?G—£¥\?P lâÙVR?ïÕm–ÐP?{ý»+Ÿk?d/¿'yÝ?t#A¹Ø«û?f±t©5ö?o[¢L]›?ïW)Ë?ƒUWF‰B¨?€z[Ò8?vwZpÇݱ?‰¡ß¸c‰?|
þú_Ž?ï÷uÓeÓ?b}·4[Đ>é–@¿÷ N?—ûƒºäJ?Q¿ç×´j¢?bcÂòíìÃ3FGL J1506.4-0340@v,ï~=Á@F•´¢3œÀ:$³ÑSDKÀ;}fÿéYË¿Ùœx,r¶@
²…-Hc@ªyßêᶿà¥ÿEÅÜï¿ê^k¶Œ·¿àÑ@ÃzÏ»¿âaZÿUNASNone?ï|žus7?"ðé·XÊ ?[ïÀ âÚj?aӓ­P3?Z^†Öö?"Ç"iO?ï›@Rá?dk%i"Í?{¼'ˆÒ&?ˆg?èu5?vµû×H½F?z¦ëµÛ#?íÈ|ˆ`Ùð?™G³Xw9?•‰ûOçŸ{?‡>Õ_??¨³9Ñþ'F?"pxõyüÊ?tÇÎ?˜vÜGʜ?bÃö~à¤Ê?a;ÃSdƒ?¬êæPÅxÛ?˜ÀŽM(3FGL J1506.6-6219@sÞò<ÈÞ+À¹§Áz‰3À9g´ör2À;¼(ßó¿ÔZë´æÉ@>—Îé2?ýµ¿©M¿ï»;µÀó?á<¶(Æs¿Ýª6˜K‹¿ÐQ¯ÝJ?âUNASNone?í$ò"¿"?²Æ*x»q?…þÔF]°?‡†Çߔßè?´7Ïy8%?±Èß³m`?ì~,ºå³h?Å×fc¿N?ˆŽrl˜Ù€?žÚñÃ4qL?¸üËÛ?I"?ÃRqCná[?ìQeÏ¥œg?¥Ø¼$?Ý?Ÿ¨ÇìOú¤?Ž8îZßq?µŠŸ‡¿?¡â.[6g¬?îP'Y?œ2?¢Ô*ÚÜYœ?i«ˆ
<î'?jT¬Ý|?©]!ëbmÿ?¢žQÃâp3FGL J1510.2-5754@t›'·þ?À›ý6¡ý–À7Ûx\2/þÀ9öð{þ~ ?âÍ'æxð@™3& !@'qàBŠ¿Îh›!%‹ø¿èˆÀa•­b¿é8©F຿è"x±OÚUNASNone? Òîð	Žæ?žGٜ¡E?ÅF@'	?ÇXTà§?é¯ÿ€Úä®?Ȃ'@î?—	kØxÊ?¦ô$ÓÇU^?«ãÙ?/4-?±\|Ÿñº?í‰J ®Hø?¶ÝŽ|dÌ?¹¨T?ü?¥úz¦BrY?Ì<ŸÍè¶'?´…y%‰b?å»Í|]îx?¶'쑥?Æ´uø;?¸†&º'†? 	šV¨?•01AN¤É?é}BÄ} ?º0:ú¾ê3FGL J1512.3+6622@Yò¬![š[@F•ÿŽÀùÀ:ÏDÁ~À<,)d}XÀx½VQ@Œ©-oz@Ô UŠ÷¿ëÀK÷œ¦Œ¿ÔÖr@Aí¿æ»™i{¢@¿ÙL…Ç2UNASNone?ï½¹ÀtŠ?"H4^?Þè¤Þç?"03a8Y?4Cr
½+Ï??ZS⭝?ïÑü¤jބ?yC¶Å=¾?ex,¹Oé?lfæÇü´À?häãhh,»?pµ±
2?î7sùqT?Ÿ}
k˜­Ø?¤tw½?ž©ã:þN?ú´ÑWÇS?'Ù_3¤»š?ïöƒbœˆ?T
K¹Ðé>õZÆេ?O²c[Õ?R£ÒÄ×hš?Säÿ§xÊÅ3FGL J1512.8-5639@t‰ÞÒ?ðxÆj²üAÀ8«l)ôÆÀ:y*GÒ&©?q»I*ß@X"©Èeà@³J'Á¿ä7hˆ:ݳ¿èc#ÿõªM¿ç®Â¾+g¿âb¨ÄYážUNASNone?ãŒL,"?Ét·Ÿ»S?'+nՑàÕ?†…BÝâ²å?Ùe‹ðúhÄ?Éh…CÏ=|?»²ó'S?ÃÖm|bõ±?—uIﱟ4?›ðe'¸¹?ëÎrî?Ä3írã©?Û¦Ç3ÃùG?·×d¯ùô?¼_›­ƒV?¥oÒ	?Ý5 åP¥ä?¸ZŸÖN?ç㕚r®Z?¶µ³Qã¿¿?dC, áÈ?cä½,¶pI?ОDÁa‰?¶—›Œ30²3FGL J1513.3-3719@t½Ï€Ü3r@1u)wȎzÀ:Ž»üÊÀ;¯=×Ñã?'{,¤ë@¨>?úõ¡à:õ¿ï£ŸB"¿?Ə`"¯ì?Ô?~~¶¿àMÔ)–UNASNone?ïúenåT?Bo¸†K0?/UeÜûþÍ?,íƼ>c9?=)Õè÷aä?>5êĪݝ?ïuá1Íô?"^·¨=ÚÛ?x'w›æŸH?|žz®,ÊO?†>ÿå™3ˆ?»6¢4Å?ïK¬ØWô?c†€–÷w?€w¿½`ß?sâ‰ÔGy²?ŒÆº
,¢+?xLJM@s?ïE8 ì=?œ*ľžŸh?]A¤"¾+?j–ˆ¾ólB?›ƒG1™<T?›¶–ž	a,3FGL J1513.8-6250c@sædobÀMݤõîÀ8SŠÁ'À:Ü»ÛãÁ?ÜA¿¼Ý°9@?' *læ@¨V¿ªOt¿Ôîà·ª¿é"K"W¼¿êª{GZBÓ¿ãìÕò]UNASNone%?éÂhH
Pž?Áê}q6œE?°A&¹ŠÖ?³0:%?ÀÕÓLmø?½Gn@Íw?áÆúpNëI?ÐϠ{?²³ Á!c?±N­uÂ?×ÅBïЯ?͜"ïB?{?ä•gr?·n˜¢æ)?¸@ÌBÈ+å?¢#¨@'å"?Ѷ¢!!Ê#?µkÅøØû?áa1+¾y?µœTfñ?ªqÖÇîò?£Wv¡Î{@?Ùú¬Ï…/?¶F_Ìg^3FGL J1517.0+2637@DD¾´ .@LÓ!ž¶9À:֖»˜ÇãÀ<®U¿ôŒ•YîÞÅ@
Åë Ík@ÄÕ"?ïÿ‡à'/ ¿ëÿe8Çz[?Éc G†¿äO€ڋkUNASNone?ïòoÊ$
?ƒ'{µd)?O*á¿wDÓ?ƒ¼—‰j¼?Gø…Û?^M<®hß^?ï¸hw©™I?…ÕÏJ;P#?qŸbifxF?x‹d6?®?r,aÁÌã=?}%(Y¬AŽ?îžq©Jw¬?¯îVeC×?Ë"³éŽ«?†-bPñž?›f7"Ç{²?ˆ[Ĭú>ê?ïJ3ôâÀì?–\•¿†?0Á¥"§??C·Â,ŒCi?–vzÍUF?–K®óoÍ3FGL J1517.6-4442@t‡JB®Ñ9@%›î=_ÜßÀ9^dµ—&À;=_0Ϭ?ßÓ-‡ç@C÷¾½ë^@²m¹¿éBÚx1¿ä[/Õ@õпèhÁú®(ê¿íÿ:Ó*UNASNone?ç&^˗Á/?ÄåeH¾ê­?Ë&sqh?ÂÐõ`¶­?°€è¼´?¯­	³)§?è̦$ãã4?ÄUhß8GQ?µ'Âìò¬?±¬Hß=õ?Âõ÷2X?ÀTâW*%¬?çßz|ŠÉ6?²:0ˆá½æ?ÃÖDUFL?«Ñ™Fhïn?¹W£q™´? Ñ¦¨NE?ãS¿k¦0¯?­'±ÿP0%?ą$ƒOàb?ª^Þ?qi¯?Î+ÝÎ\ã?ª=êq 1F3FGL J1518.2-5232@tEš¿4@‡;…èíÀ8ÔÜޒÇîÀ;ëÚ¯
Ÿ?ôèøo"@ŠìËÅ»¶@îÿ´€¦¿Ý;|Râ¿áhʧ·?¿âōñÎB¿îìӍ†:íUNASNone?½®0™ã…?·k}Ë?çàœöÙ‰?įø|½%?Á¦‹ŒNø?¾ˆÊÃéf?Ì{·¹^Ý?Èj7Ô\zò?փ"ŽcW?ÇÖµÚHr?Û>Ÿ•
B:?Ëk–ÔÓ¿?Ôd'¥e¤Ý?µzÙg²ü'?àYꂕ¦?¶ðÌ ±?ÅÏ2ªàs®?©z;JÃÀ?Ô"ãŽ>?±–©'ÉC?؜'i2±Ï?¹!
I"`?Ó@‹z??±`ìuÝîj3FGL J1525.8-0834@v,)³ún@C%žYò»À:©Yš¦	À;²X'hLð?ªf€‰@À—µ=å?úM]ÞØh¿ïÿܬhÔ*?ïه2X&?ßÔUq{¿Û†fÍz­×UNASNone?ï÷ÌË=w€?^ðª-C?8Iã…ôZ?Z¾HúÎO?D§áG(4?HBí§"x?ï¥6våÇ?!Îm_éš?wë–ÖÎÚ?ŠÔ"Ê#Ê;?uy-¶¤Â?|ñ
sÇ^r?ïEŸ"
ð©?"9±ª `;?ƒAčۑ?yÈKJ"	ý?‹VZp1úD?yk©yÌ*?ïÁ´pâ?…Èc©kâÂ?LLxaƒ'×?^ð¿Û¨´?{œ8'Â	‰?…&®ä¬ñ!3FGL J1526.3-4505@t˜Éšé$ò@#Bö@c^À9•xgðª"À;FKMÜ?Ú…`I
]@¥Vôƒu@#—Á¼M¿é—Gý¿í[ÌçFB&¿ÐG#H•¬¿Çh(ˆ¤UNASNone?ïk€)3ú?®=iôó–™?KD:^¦5?O'EDR<¼?'µÙދ‹?®.6¤¥q[?î¯pA;¡ä?¬þ¿šÇÂ?r¹lä׶?{M>¤øٔ?¢±ÎOÅÆÇ?«<°d‹D?ìíË--Å?¥•ç'è?»[Œ‡í­?"2>ÖHû¡?´húÃt–n?£rci;<A?í°âJ""?¦ææ߄?EóïüGl?Vø—•÷f^?²MÐM?¦Ý6¡3FGL J1527.0-3804@t܃ä%¯@.¤ÎóÀ:š'Í¥:À;€¦'F•ç?¦oÑòlÎ@6žK…@¡í`@1ž¿ä†¢Æê¿ì'Vv{ª¿É€@›ëGP¿Þ°4|UNASNone?ï$‹3µ]¶?§ª˜;±t¤?@ý©ë¯Q?Eb°oÈy?šæ¬9ûKº?§~b6:U?ïNúÁ.™œ?¡ËæÍVr?p0FxEFá?s®Ø-"c?'–<zÉ?Ÿ±Vñ5•?î ,V!Ýè?˜òå7q6L?‹L^þã{Ù?|¯#-c"‰?§*"Þ)B'?•Š–/,?PÑð?˜ÜÜ~¦»&?HòÂ]n-°?S¢.¯•'?¦ó?ö(D?˜³˜÷aj3FGL J1528.1-2904@u9ßý`é@6m
$F0fÀ:ˆäö=öÀ;¡míCdÚ¿ë;
ª‡½@
–cî<D?û%÷@=ݱ¿ëΜ¡n¿ÝÑäy;Ö¿¬¬àÐ
?¿èº³Î,UNASNone?ïÜ6º·Î?zËGéI×	?UܑDZË?_kÄ,Ÿ·ª?hÚüd±‹G?w	ŒOVøA?ï¶À—ØR?"€¡FOq?k'ƒ<g'?nÐçm°w?w1ru£C?€¼¸oþ
i?îªÞƒ×
?–~í»'ò?'ø³ˆd?‹ÙÑ{uد?˜¬Ò7ž?Žrt_Šbü?ï\A"˜T?µ÷6æM?+^Æ^ã?6Þ$)Ü1?"AÚðݼ?¥¼L1%ƒ3FGL J1528.7-2247@u€Jßø"¼@;Evš'^À:™ï)îçÀ;šXKñp?èÁǒ-ù@
ێ	Ãx:@ðßëb¿Ùz£QJ¾¿â-J¹6Âà¿â™3ÅÕ6Ô¿ïÿÆ×âYUNASNone?ìa~è4S·?¶Á(_X ?µ³*,?´MèRœg^?zÃŒÓ?œ°ÌQýs?äë VX5?Âъ>˜Ç?Ò0ƒÛfæñ?Á
X®…@A?¯ÉÛ¿EvÑ?¬yv¸¿œ?çâªv"C?±Ê¢ŒÀ(?ÅTý±Oé?­JÑH|[e?¶àSñ>?¡ªœ¥?áÆ3'¯J¸?·ˆÜaDK?Óg‰:çóô?¸	Zç[ÓÂ?Â?rí9?¦ÈÚ·3FGL J1529.5+6733@Yß1)Ë«@EŽ'_ét£À:ÄŵV­À<3r"XÀ¿ëg¿p³@;P'¾N@å
ŸÁ%û¿ÔÌ!nî'ï¿çnéÍíî¿ây|ˆD¿àÕõÀêtUNASNone?ïɦOÆ<Õ?†üÞ\Ã1?uwDü¨!Á?…me³–7?VÖL€åÐ~?_Œ!%'üä?メb¢e?~{¸Û7!<?n‰šgæо?qÁ,PÆk?qrzÄdÕ?t9j–s-V?î!ÅB¿›Ú?ž' "t?¤;õŸ-Ìã?œôýuQb?"Oli°êü?'*øB¥?ïÏð@)ÑÃ?t0fB[c¥?1^ö
·6b?2ÆOŝ]?vñðŠ;«!?sØ4•¢Ÿß3FGL J1532.0-2618@ucblvK@8ºˆ&«À:#Š·~‡À;†@Ú»¢Ù¿Øp™Ã@ú¯Åüe@uí οௐæº9¿â(GŽMÏÛ¿àç¡Ú…È¿ã¥1 Ö²UNASNone?ïÛMxN?Šçî¨m!?Tõêa.œ?'™ü"ùh?jz0'c?_i	?Úø?ï°rÎá.?ƒ	V?G3?pÕ
'f¸?p`øXš??w°Ã"×'?}7tf4|v?îÊìjG·?ç":™¤?ŒQ.¯XúJ?D¦ò|Ëß?˜yÛ_\¢j?†øçÇw….?î·ä͏¬?l/gÝ?\Rd'B;?Vɯ²Eð?£Ÿ {.§?7ÇP‡3FGL J1533.8-5231@td <K	ê@"]¶ŠÀ9m'Y4À;
Vìu߀?âÎApQ…@KšÌ>‡?ÿrû?{ëß?í•ï{«ûz¿Ù˜Ù]Ý^¿×(>;é©ì¿åŒ2 2²UNASNone?îfD[á^?«¯â³Kíú?">¶·X;?ƒñùVVR?¤Œ ‹Û^?©]çqËU?á—ä;íÀ–?ÕÈœÊ"Ù?¤•ìŠ¼–2?®l×!'~?Ú=yöÌì?Ô£yë'ü?ëÙ,T¤ñ?©š[ړ('? XŒ€ø?™hƒet?¹+®'6´?¥¸Fë³=?çN¿_ûF3?¶F[xO?›cK4œ€?'íƛ(¡Ï?ÏX™,S¦?µÕ<HqÞB3FGL J1538.4-4656@t¢þÅm\û@¢—žÖÜÀ8•;!>>)À;còPë?ìºO¡þÂé@Ë­MÖw›@˘¿Ô쬿èo‡]"V¿êúÌ5¼ê¿ê"Îà¿ïÿ¹€Œ#ÝUNASNone?ïüšTE5?ŽnDdCÀ¿?xÃaǾØÁ?"dëk/Z?x>QŒø?€œñîÿ?Û!¦ºÜsM?ËÑÏãšù?Î÷ýR²ôœ?Ân|;p%?ÕbZ›Êe?Ê<å^è?ê_^+À'?­ñ_møߜ?µ3Ü Yþƒ?¡ úíNL?·ÔnHG?¤;¾âó]?Ô:7à™Eâ?µasÌ×´?ØI"\
õÖ?¾—´ä'?Ó|4Ã[ÄH?¹dä?Ç3FGL J1541.6+1414@7­ ÝD@H2`=WyÀ:eøg…JWÀ;¯ëí#"j¿ß±‰ñ—Å@
#Ïj¶Ø?ÿš¿5Š{¿ï §IŸ?íx‹dw£Ð¿ãW}vö¿ÞÈfžùœUNASNone?ïñaä|
Y?e¡üUd'?@MéØÕ0ù?B5;撗ò?UBz´£?aÅ|œèØ?ï†Óæ(–?'et…ˆz?'C —h?™s©Îh?xoU彖´?~Ê\–yô?ï*7jŒd?ƒá»É=BT?"'»‹
?vŸ(Þ ?{»M)d?{<àÄvYª?îåBêÊ)?ÆŠ<Æv?—±ŠíJ5Á?šl¹:²ˆ?‡L/ráT?ˆå¤U±^3FGL J1542.4-5911@t4ÿ'+¾ËÀ
-\Äüô³À94If{_À:蟔…]¢¿ë—7'js@2·7dE@Ðà©-`¿æq-ãÀã¿å¹û6(¿êdV#Ö§u¿è¶u>_PUNASNone?ëO¡¾š$?¾ÊÒìEÖ?«hšƒ'ƒ?«ñV©Ìó0?·Î¤Éd¾!?¹9xÚ#?êÝ/ɸ?Í&èM…?—"5ê"j?¨µÁh»ßÎ?Ī%ü‹Û?Ê5ý¡ƒ8ó?åð—W	9?¸·J»›N?¶ê^µaÌö?£d"-vX_?ÌÊnGòô ?³å÷µj0š?ê	ºnw?´Š§ÊÆà?rK‰†z]?vÚþãnËX?ÆñPâs9?´V蒖&3FGL J1544.1-2555@u‹ÁÝ!ê@6œŽ:!dÀ9/Ô!Tä^À;Y 8ð?õ'ÏÐã1é@qɎ~ÞW@Þ]@L÷*¿×Û«Ë(œ¿çêeÜJ:®¿å¸y™§¿ïÿ§¿!>UNASNone?à?–'×¢û?Lj7]@?×âÓ3EÃ?ƌ¾ûͤ¨?¾wþ¤.y#?ºFã+§?ÍôÌ{?ÁÕþ‰r¥©?æ>+ŠëÎË?ÃÓ¹ÙÅ/?³ðºf"~?±Bñ'÷×?Ýp*-~!É?´ý¿÷
q?ؘªöOQb?³Ž´®…Ã?ÃîU¸e¬?¨vÀÌÌ0)?Êfâñ•¢??ª¾ä`S§^?ãüò2s?¶…^ãâ?Ŧ¨–¡"÷?°˙½3FGL J1544.6-1125@vC`¿]x@@~Àð¸À9iW²n}À;Jǘ°eŽ?õºçG!}@á—YÎR‰@M`@1ž^¿Ájàܷ"¿çà–>¿æ	`m?¿ïÿá&Ž4UNASNone?Ô§ÃËÃ÷'?Èa¢^?ãqßb­¾?ÊKß%´?´­aÕÚ´?¶ÆçLBó?· tôYž?µQ«é`?ë)EfF©?ºã¨éó?®*¿³œb;?­)²ÎÎ×?Ù'–í3'˜?´&$Ÿç*?Û»[ZÞ
?³ýI40u?Æ:p] ¾?¨#b½bX?¸Æ6ÇæW??¢A®·~«'?èÐÁºÍMò?´'nÍûÄn?ÀYݰל?¬"ªÁ›¼3FGL J1545.0-6641@sîἩiÀ"Á'Ýãu†À:'Ns*šÀ;r3#Bû?Ñ…cñZå@ûÉTrH?ú¿æŸÜ©º¿ëÖ€BÓ¿å"x†/Ú¿ª5.é€k¿µ\]è­AÜUNASNone?ïë{•·´1?Œ"2—^¼š?Ïâ1 ¢N?Lÿ½@¢¶?cë6¾ÉE?Š¼Tú¨L¨?­ÉD?ª#{y`?m¥ÛMjR?w½JT "?¢=w}®•?¨ZAvð"}?ï2¾›F{?ˆ½¼¤¦Õ?|*ŸªÁKâ?rA)^™?'"¬Œ½ ?"*9\•Þ}?ï£bA$2?%6S' ?õ1ÇF
?(\(ê:?‡…ZÏe.?uâxf83FGL J1548.4+1455@9¡ë¦¬§"@G–a©É"À8õªõâoÌÀ;g8¿E%?Ü26Âù~ @Ø"´Šá›@å­_Ÿ!ï¿Î¾¬ÒË-T¿á™n·©á¿ãJŸfy¿ÝT{eY©UNASNone?ïðûHÀðÝ?_ۗqØn«?G"Ó"#͑?Rþ®ôÔö?R?´Œ^?VŠý
,âI?]:Ò?‡€ï'>}?zåÜ'}]?Ñ€é­?vLõOeä?xY¥Ù?îßÃAߓÑ?'jp>ä±?»›,Ù?"ÛwbÃSá?•"9öw"?‰»Oþáö?îšãˆÅX? †ûUgŸá?…ç´Ánú?'ˆ>"²‡ê?©´WÚCNÃ?ŸÄFøÊsÕ3FGL J1549.4-4832@tªó¡LìB@ìúi¾
À8²³8§{À:ÑuúÔG¿é1©´€@~A…†g8@ïš@]".¿çòŒEYa¬¿íc\‰ÿÙÑ¿Ó«›q,Šo¿èp³hÅUNASNone?ã\äHJª?Ðõ³éÈE"?‡*"åâš?'¤Ü;E¼‡?Ù>ÄãH;˜?ÑSÇrì?çUÂ8ˆÈ ?̼€Gú«1?¢.*ÿ.«%?¨U^ȆwÒ?Îl^2·?Ê9lf®•·?á	~k†ý?¸^œ•'£V?¶½…"ôw?¢5™G@?Øf•¡Ç´ç?·'ÏÏŸÆ?à"4gÿ:?Å.ùºó÷?z—ê&S÷ß?€ÖB<€6è?ßQ7<–±¬?Å@ÜÝöî3FGL J1549.9-3044@ueâ'@·€@2$<µ¬À:f6ýÃÞÀ;"¹
Ó'Z?éÞ~š²Ý@€n1áÏh?÷¦¿òÉ·¿îm~ÂÂ?ï÷TYb`·?»áéû—÷"¿¡Å«%.ÏUNASNone?ïô'B?g|ùàÚ5?BØ@(?{{?G%XÅ üº?JßSÒ¶Cþ?dÌ®—˜a?ï¤>Ó ß?‰ÅÃ#Ü/?r3¸?\ªŸ?{.F³!o?{Œ¨VÒå?'G7í݉?_F1y?•|w{Ç÷?'–7 ?Šz;/¼?šš½R?Ž¨¹¸e)Ê?ï.ÁP‡æN?œ¼J¾<‰M?xÎf¼¼?ˆÄ7¢3>×?"ô<?ÿG>?™¹æ¾H'3FGL J1550.4+6027@W^qŸŒ¨@F‹ÙÂ~•1À:TcûRÀ;ïèwM>w?¬cª²h@jùÀöªÂ?ýƒ˜ Õú?'Wÿɸëû¿¼!`DZÅ@¿Éb>ÛÕJ¿çW
×ÈÃUNASNone?ïÔ¼ƒý¨?yªŸ)¢šF?gíf|œœy?rÄ]3¡¥?cV†\¼~?iIí·HÒ?ïM‡¸R"\?'Ãh7áná?ŠÂ0PùùC?‹+Ó²™–¦?Ûáša/Œ?ƒÀicq.?îÇXò<ç?'Ó–Ùa*Ô?'ux»@—?‰hè÷ÊÇ}?"Ÿ†¦wÌ?†,`ÙôÚ?ï§~n
—?'‡Žã4?ÌÌ­€Ž?}$Îï¿Ä?"d©Û»lã?Œ·›øÊìh3FGL J1553.1+5437@Ue3]$žE@G•¶Ü gÀ:&¤¯wÀ<y_gn¤¿åZ¢ÕF\Ê@˜•¸Ž|@
eÿ¹3=¿Þêø˝¿á÷d¾¤µ¿ä]ql¡5¿é©Ïzã1NUNASNone?îÿ.1ƒÉ©?°o±«‹e?›tÍß%a…?¯mPæFì¼?r•¯Á…¥±?|™íÐ0?ïz»K2!?âwõ.¸?'ÂÔ<ù"?†3wýÅ?};ø±ìüX?s6nk"Q?î½­òf?›ÇÛ!,	?¡xì·0w?•/'-;½?špÒ­òJ?‡<œê·<¡?ïr²FÛí³?ŠEéûz#è?q24&Q6h?rÀ8öv?ŠºT5Û÷ß?†3Â/ªp*3FGL J1553.3-0322c@vñýÞ½@BJ^Ý)5À9mlÓgñÀ;Q'TPº-ÀYsä©7@Zž¥òîJ@€p]¶¿é2ŒÚø¾¿ãå×;K줿ì2©J€q¿Ä?"úÐÐUNASNone!?ïQªÊ¡Ù?˜ûß.Nÿ¦?…Þ®ì_æJ?Š7AIX?…à¦`÷£–?÷®I)º?ïÏh¯)5?'û_LÁ±Ë?b|¨-ý9ß?hŒf>%"®?n¨¨ð|?€ÏvY,më?í=±BgȾ?ŸË£$17þ?  Œö»ª=?ùó¢S?¬^âÇÉÝ?—{Rï]?ïÐčVÿ?y°W÷¢…ß>â"—ž¹Ý?ÇߖÑ|i?w"¨±!ñ?y¬1ʖ¡3FGL J1554.4-5315c@t"Ùè>B[?Ö-íCdٞÀ7Üݸ­[À9Øró<£?òí±ÔxèŸ@76³t @
 8ð?ÜÖF±rÜÊ¿ÞGh¤¯!k¿åZeCё¿è°Œ'ãRUNASNone0?iÞVðO
?cþÕ5M´?¹Í}Ÿ};²?»x³Íd¨ã?ì¬qõöh;?»¸UÿºÃ?w+K±R•Ñ?‰Æ(É?¿ZÏuV?¹h£hfz?ëñ>®¹	?ºÌÁ!êS?§"ÅZP‡^?";#Ðd¬?Äú8痠ü?®{=T ?éOEpuK?¯¹ä«C?¨WÏӇ?¢Õ£Ài:?Á=I4HX?¬XýÃGjI?ê.ÝH5ð²?´Zš%²î3FGL J1602.8-1924@vç#$È6@8Oh7÷¾À9Þ_>Sø¦À;eéÁЈ¿æcÊ«Æ~@l˜Œ´Y@€õs}¦¿ãþö,RÕ¿çIQÈt£k¿â6©µF¿äžÙ—UNASNone?í^×DL?·‹Z=Kñ?m©P+c?k€'î/?´8•TDÑ?·.öܾ
—?ï±^e^?'œ¹m/¬?oe'¬óþ‰?p›ƒÈ?wž2âÓQü?|€—\g*ˆ?íáÁŽ'Ü?l.
h)?'[œ3h?'ðwìª?¨âÖeɸ?—ØKF:`É?îU+Ë7›?"Š]·&/€?S…í"'¼a?PÎwè¼iÝ?ªßéÀ3?"Wݱ(q3FGL J1603.7-6011@tLƒùdÀùà`þG™À9è¹/a›À;k½"J¥@?ôèâ'Äb@hScTc/?ÿeþ>´Æœ¿äتÐgzÒ?äÖ©G¿Ø&ã&³ü¿ëMãÃçÔnUNASNone?ǜ¾1 ï?Â\;¯ãú?âÜ26'F?ËcS[a
?ÌóäôUú?ǟe4š(?ÅʍNÑK~?ʟ›"…Q?Ýá­º‰4*?Ì·îÆ«G?×9ž&?ËhI]Ð?Ö60òØQ?·ôY/°?ÞÿÔm#ïd?¸Ä™‰֏?œõA®p–?­*©Ü«t»?Üg¬Òdw?Ãj¯égv?ßIŒc‹÷f?ÄS>%ìÖÁ?±=³¾†‹?©Ü|°×­u3FGL J1611.9+1404@;ÈnÁ~ºñ@DфV!uÀ9ÞÊ#¥ ¶À;¨÷ÇLZL?â~M±A^£@5»Gdâ@­_á'¿ßTû‹bZy¿á˜'xñ‹ý¿æÐB=šÈÌ¿àÇB+@UNASNone?ï[oõc ?¡ñ^^:aë?‡%"H‹?Èº©>3¾?ÿÏQ¢?žlž 9?ïnA³‡?þXù;½¶?"LOVž!×?‡'Åa?€-à<<?€S-Dr?îƒ\i/\¬?•¬-ÐÎÈ?"ë|"CY?‰ìh&Ýg³?š©Z]'?ŠÄ¥£Â~R?íê¿T"t?œ N_É?•çx/@ä?À!;rvŸ?¦`NŸD3?˜)pä/ðß3FGL J1613.4-4222@uû_ïJ@t‹e#pHÀ9p¦]¨À:óˆBY@ä¿ûÚOÊB®Ñ@cƒ•vI]@zs 
Ìã¿â,3_%ª¿í— m‰¿Ûš+ošl¨¿åÁü¸‰1UNASNone?ލŒá˜Å'?Ðл¿(ðø?aÍ_Ïö¾?`Éã,p"þ?à§l/dŽH?ÐÓ|©0¤?îõòb?³ê*…îÆi?op1b9ÂÆ?vNK‡Y)?­IÃº²#?³?¦a=¨u?åáIÅfËÙ?¹#¸½¿?§§ëV—?˜ƒÍì?Ñ\·wÎý{?¸	–Å(b?í:·¶Jò/?ª´}V¶??»7˹Hs?!9†<¬U?¶$Sµ€4?ª±û~á\93FGL J1615.6-4450@u*™0¾@?û¹IbÀ8Ó%žõùíÀ:³ËE
PK¿ì@†÷ð*å@Æ4/²u3@~ó€jÉx¿ë`ûZ©Äµ¿çÒí!mc¿ã"T
"¿äÝ
ë-¿UNASNone?îò«°ƒÊ?±(åהû?o҅Po?sT2¦}Ïä?­?è¥þX?°ÒûDz¹/?îqM…Ãûº?­ßcEj×1?lâÍ·bCw?zº•<â?§úÈJ ?¬°³
Gëý?å=l¡¯ÓX?¹'Ã<Ë?´÷¢¤üs?£Íùëv—?ÐG>9·3?µíD€Gd?ë°°Ø°U¦?°S~	‰ÌÝ?B#˜L¶æ
?CþÆoÅ?Á+ñò?°K$Ò;ƒ/3FGL J1616.8-5343@t§—¢H"ÄÀ½Õü woÀ8ZÉX¤À:ªí"Ãq?äèKË@]ÄKžäÝ@=Žà-&Õ¿æÔ¾+Qðì¿ãy9Ó>­¿æI"܍¿ïÿÍݐ`ØUNASNone?ÎK$jTâX?ÄZé19$?Ýk²`ú,¬?ÍôɵîÛ?Ón»iÛb)?ÊsnÇ2^?¥´ëҊçÇ?³‰
45[?ß<öå1ñq?ÉtèåõÚ?Þk |±—?ÉiŒ<"€a?є
NB?´bÍ;s&?҇âI[j{?±!MN7©Í?Ûä
œšGC?¶Õ%n¹¼y?ÆÇu¶¶)?±ÝÉ®Ú2?Ò¡zY­©ü?¿‹µä$K?àýeŽ{}y?¿•ÎËúK[3FGL J1616.8+5846@Va
xÀ@EX¤Ò²ÀÀ:1ùˆºWÀ;ÿ1æ,?Ï¥#\óÃS@ǐ:`˜@ʅ˿î'ßÞCå¿âÆm1ܛø¿ïü"±Òæ?ïژߛSUNASNone?ïßìn¢Œ?"¾x͚q?iw~D1?ƒÇ.Áu†?JpM(¾Ïy?c—'—và?š—œ	?¤=—xÁ:?y/f™=‰X? l¤1_?uLôq¶?'»@ƒ¶kò?î˜ëedR?"âòpáޒ?"Ê'Iã?ŠÔ'²*÷¹?™Nns?ˆPS7n?ïÞà' 3?}qœ.µO?H3⣶"h?eáéÊ4´?kuVrD1?z9$Ñ['W3FGL J1618.8+5520@U:rŸYÌû@E¹¿ðEwÙÀ:·!†b…0À<(‰hÉíõ?Ûrv¥"ä±@n@'â@œ?ÿIw¿áðÁ?·¿ãô™'ì3ù¿ãQ厾I¿ïÿo•þÉ8UNASNone?ëúT>? ?Äù,™5G?½Ù쎞ë©?Ľ©Yz¯¡?'›"ûxÚÉ?‡8Ž7ä"Ñ?ãÚrD¬l?Ë$êsN ?Öq ݓð?Éõå†'–à?¯>ÏÔșÇ?«o"ãÛÆ©?éßo%.Γ?²L
n'°?¿Ÿwˆþ.¶?±	Z'¾rÞ?±eM‹\¨?œ®\êy'ç?ågW%o?À/ZÇäE?Ñ}¡"Bz?¿š¹Á×÷?­""õ>'?¡Tmf83FGL J1619.0-5014c@tÒy»­À˜?Ÿ¶a-ºÀ7á€hp+âÀ9©{rg%©?ñÂC@–ÕU‡pø@s|‹5©¿à2׶=r¿é'¡˜Êr¿èíçؘ¿å²8]$ÚUNASNone9?ƒÔþ#Sî?‡¶Ôfå<?¯žŸLc%?¸Hn=ìAþ?í¶Å‹A:ž?¹—§°$>?©I¶wïó?¶VNÁ!¸?³K{€;ö?¹P|Ì"$!?ìõ(y'?Á®á¶&š?ºzÊ2Ûª?£…SD?ˈӡ]ÔÌ?²¼5ñLE?åÛ¾b/X?³è}W<Áq?¾RÃþØ`?º6M«Nò?•G©%¹ç?'euv '?ëeBõ·%?»u6á²úÒ3FGL J1619.1+7538@[EÐ|"µÝ@A¥ïÝëÙÀ:ԛÀ»F"À<%ZÞrç~?âÀùɞÞÂ@~¨Q˜?ûg€)†¿ïõÜíù›?îã†tù§ ¿à"m¾‰-?Âs¿Æ»!UNASNone?ïàëXs?.щpÈ?kT |ˆú?$(ã§?>áX#¾¦?=/™¾?Ÿ?ïÀ®õ]3?€ÓÀKߌ?n:oI•¶?w=y'j¶{?p‹¹à†‹o?ṡμ…û?ïð8®©]?'®hGF+õ?'ȝU4AT?'ì¶ÇOÂ?"r·)í&?rïÞ Ü?ïÕMªeCÔ?}æ?C¬"‰?j'ª<jQv?y%Buˆ{?`Š«^QÚÛ?k°ºÕݺ…3FGL J1620.0-5101@tËa\¦Ê¿ä?ØÝý ÓÀ7çÇj<"À9Éb¯ø€°?ñÖþí|l@_†`ÔV@[€YV³¿Ôꔉöt¢¿Ü{õv[žY¿çÎ3¹¸?n¿ãf1R2|ÕUNASNone?€4"­©
¢?Ážé
Í?ڕZåc?Ñʐ;3¶X?âtŸÈ@i?Ñŧ	½çÍ?¤Æúò®GÝ?±õßöòC?Âùÿ49rY?ÂfÇæ‡?éõƒÆ¾ì?Å@§Î¸Ê¢?±}êH³`?žMéV?Ì?›†2mj?³ÌÂw©é?æÀ[ÕoŽ9?µÐ/ÂÙú¼?¸än
?³À*YK‡g?²%hæÚÝ?¨où:üfR?ê©Vr ƒ?¹S…¢¤™3FGL J1620.8-5149@tø}¿H¿ô™@
6IhÀ9
Ñ­ÝÀ:oê3åàš?à¹+¤bd=@™Ä6%@»Õ@Ž»o¿ÞmW°¯Ï€¿í!]'澿CD?S)üT¿åµµAüàÍUNASNone?ÂÑbµ¦au?Â@Š1T­q?hOC"œ?rícDê+?ë3–$?ÂjHUÆ?Ë	¥¾n¼?ςʑTÞb?«ñ)Ä‹Ï?²¯S¥	?ç~‰zO"?Ð ˜|âÚ?ÕK`ù•?¸äœeÐ?¯îMÙ§Q?šW83k³?ã[k%šý?¹:ďR!ñ?áÓÀN •ô?ÉäϾ éñ?]€oUT?i:¬=¡"Ó?Ü:þóª?Éæ,Ç3FGL J1624.2-3957@uQ¢3œ¿@–ž^$x…À9 €©ÌÀ:³À~à°¯¿ª´‹P‰@×´>ág9@(‰ðü¿ç"[À×1f¿äEmG¿æ?d€¿ïÿá{ýɼUNASNone?ͦ32î:H?ÇJ'F¤Ë?ÎfNzÇ?È©A͘Rè?àü럿Ҽ?Ð?¿¯§t2?Üݏ
Â?̺×äÿ4?ÇÞB'Ê¢?ÁÀÝU"þÜ?×3Oáv0?ʬ"W¦¶?×3àIòÊ´?´,"*%ó?Í̺~b"ž?®¹,…=œ?ÙåÂvÛòý?µJèތµ³?̈‡,q.K?º2@ä¾U?ÄuaÌ\¨?¸/?-ŽÞh?ãÀ…Áã]D?'¼@Ò]Å3FGL J1624.8-4233@u4®}Vlô@…`&±EÀ8ËAøÈÔÀ:¥Zs¿èʔŒ6@2ˆ9tëº@:×@H÷¿çD"8­¿èCÂöÆV¢¿æxþH𴳿楿l¼íUNASNone	?ç‰÷N\På?ÈÞA´€tî?—£H0ÿB?š§Üb].T?Î㈜?ȓgØž×?ë3Ìxy½T?̇Ç?…,ÌS­Ì?›*ùm?ÁÞXÞ-ò?–ïÝàØN?ß®8_RÆ¡?»&ÿ÷?¿ÄVq›¦o?¦m
à ¼Ò?Ø`²FOÃ?¸œ§ÃLÜ?ç'ñӘJ¥?»ÇùÆÀºÃ?gÉW-h?gúä ¿?р‰ª"‹?»ÂÜΜ$3FGL J1625.2-2845@uØ_ôö@,fÃb(À9xx·¡ÂÀ:ê$=Ìê)¿òôv	³@ÁþÙºF@)¾×ü¿êÔ½âvá¿é¬ë';¯·¿á»<QÈ}:¿ÓBBÏ»óUNASNone?íõú>|¬ô?¶:2ÑÕCg?]…ÇN͙Õ?aQ•±F9?¯´-ݾÄ?¶{ûÆD?ïqȕي?›_!˜q#¨?d–š8öß?p!A5?±Š?Žh3û_õD?™qȉOí?ê5÷qbŽ?°Ë½Îã5? Û³Ñ"£ö?–Sé–e]?Âñ6ÑÕLË?®ÎXÉ×Hµ?î"DkZo?›C–`N½?
5¯þHE2?î©Ñ]I?¦ÄkÞY}'?›Ê*Ùq3FGL J1625.6-2058@v:®záH@3I§;BÌ-À9EÓ)Þ À;"Pg÷`?ÓXŽ-ø@
g%Pq‡'@SÏÿ²'Z¿âž¥ñQø¿ìáWb+]¿âøLòì¿ç¿ˆOªUNASNone?çìò
ö?ÇãýSÀË?=®,ÁÞI?Œ™ÐB?ÎX\ñ[Ñ×?ǬšRï?îfõÔĎ?§'Äqû?šµ³ý{ŸÙ?—Ç—•ùQï?˜k'iòŸó? ‰Û*Çê…?êd3)Þ?¯e3yVŽÀ?¦ÂÚešs?"1U|K܎?ÂG~|ùñé?«ßå@¾é?ãZV©W*?³êž')?§lãÕ4߇?šé¬r™#?Ö]Dصº?³žAŽ¢h03FGL J1626.2-4911@tër{²þÅ¿«Ýqà˜ÆÀ8|‡5DÀ9×ôm$Ɖ¿ðÞ	îkX@PæMÒEÞ@ÚÁ`ˆ¿ç%—=$¿é«´x÷¿âì7È]¿ß¡Ìts€'UNASNone?'ë~²h?™
ڜ3?`çZ¯ö?l!«h±fà?ï_½fd?šþŒ¯2ä!?ÆJ>9%­?͌
xÃ?˜êìiÐ?£ª,Y?é¦n8?ÎTˆ"ÔB	?ÃJ¤6¹ƒ?ªá¾¯ù´?³9!ÆB[?¡»¢î¤?èÆ2Θð"?°u¿·")?ÙüÓÌò˜þ?ΙJ;`Í?-€x«YZ?3<ÔÓ£?âÿ¾ûýò?Ι–á̳³3FGL J1626.2-2428c@vð†nD@0ä^	}À8Y
×ÊVÑÀ:]$
üB?õ¡¼Ö_@ÇWC]ͼ@3õ§:A?ïüçEا¿ç@Îk!P¿ã¬¡gT‰*¿çÒ^ö@ʲUNASNone ?ɬi>Ï´b?Å­† o¾?ږê%=š?Âgt»þ?ä®?õÂÁ?Î#¿tO"½?äiëóùgÃ?Δ¿?µ"Ù?Î7©-O~?ƤO¡èN?À!N†íy?Â8Æ&¯È?ÖÇ#ëêÀ¼?²Gõ4?Á땗ø-6?§'"û[²c?à!ˆ¤"T?³8j÷J;¹?´Pñ˜™%â?¤±'"•?Ñ)êM®??½öÀÛÂJ6?äàì†F$?¿ 6º»@3FGL J1627.8+3217@Jz©?)
»@EšÙ¾L×IÀ9ÆñÃ&ZÞÀ;ÐÈ1\™^?õc\†=Ç6@úË²@=?Ñ|4?ïߞÎ.C,¿àã­±K	¿âÎ"žv´N¿ì"äΏ£UNASNone?³nۆþ\?²«q9Íñ?ìËfIÖD?¶'¬µ€?˜ÚûW"? àˆřt?¡@ñPéu<?¯ØLAt?íÇ&¾²F?µíÿqðq?¢L¢Ãò*~?§©{ã«Ç?Ï¢ ¤ïS?³žWvÆW?äOa1Àyl?¶8>³a]"?¿W²0²Uü?¥ƒ\7;Á?¬ï˜ÑvÕ\?¦©º°7…c?ìÄ°wVG1?²X´x`uY?¦Å_¹$·'?¤ÿ]?d.h3FGL J1628.1-3344@u£"úÖËS@$¼[òoÅÀ9ÉÔQüLÀ;7ò<ÈÞ?¼Ií´ÎÔ9@Ùéù-}è@îÉÿ½åÔ¿ëõŸûø"U¿ãg€¯è»k¿à)«[I8¿ÓÌȝ4¦UNASNone?îÕ5¦x¦Ç?£¥ÿÆ<iˆ?i¨£1?g8±¾/ñ»?¡+È+	R?£\áoÔn?íùFÐÀ¹^?³—û
$*?€D슨?™c
.ò?¬KÁðùGx?±Ÿ]6BEÌ?ìÚ=¦\»?¥˜VÎ<ðm?•yN)(Û?"Y¾¿çrà?³Ñ*ˆƒè?¢àÎuڑû?쬇Ǎ	ì?¨ÝbÛÎø˜?hIõiô?oYÝìtiz?¹Ùy+ïMT?¨§p2J°(3FGL J1628.1-5740@tŒŠ\å´$À"yÔØ4	À9²¥ùú,À;#áâއ	¿ÚS'nGË
@×qýÉD@¶ RÛÅ¿å@+=U¿éÐb×CPë¿èV™µ{Õí¿Ô۝Fï UNASNone?éL[ûÉ?ÿsכ!?Ÿ§îkI‰?¡Â
'Ù?Æڰ±¬?Ã܎àfÚ?ìßäéƒé=?º,ý/ÖÒ?Š–ˆÞUc°?™d´Pnf?µ®˜	˜?¶;^nÿMO?êtb{
B?®Àê»N™?¦'SÖÂ0?"—(´ô{7?À]ـc>ó?ª+öWuÛ?êÿznM?±"µÒL?d;|äiÃ×?i£ð"N"Ê?òØ"µ$?±†º p3FGL J1628.1+0254@1¥‹'¡¡@@t<òϕÕÀ:L(Àª'À;´Ì3?æ"ßÉ\]'@M÷Y¾7@ú'ßk5¿º["'0®¿ ÷?$‰ö¿êP*v˜…¿×b2¢ó9UNASNone?ï¬EºóX?Š"^="e?'džúMq?‰ªäĊ`?Q8RHôäÄ?URíÝ{Ì?ï g¸!0"?‡,ã8H?wËá˺p?|?ÃZþóˆ?xB#­mú?}"gË7ö?î@—àU-Å?¨Ád¾?¡ç®Ì;°T?˜ûV$c!?"¦\âæÆ?"‡–zçýñ?î>Šj>Y´?¢«ócn"?ŸÆ·—Š
? F.ҌR?˜gû ª<b?"éÈtÛÆ3FGL J1628.2-2431c@v(C€ˆQ@0ƒ	"ãÿïÀ8wÒ<çèÀ:dVè'?âöZ'@H÷¿>Ä·@ú`Ãd¿çp^{¥+¸¿åM#"qÑ¿è@Û¾hl6¿âUQ©üúMUNASNone0?ÛN.2—.þ?ÌñÙby?ÉãkòíS\?È$G¬¬'f?×ÀÓò'T?Ï<̖1À?ìpOï?¿}µüÛuZ?²"yw±ª?´×ÿ²Ü6?©¢
A¼?°Úh9-Ú?àO$ºÂ•Â?´3H#Úâë?ÃËßte,?°.‰£`ÕÑ?Õ|.šÀ¡å?²¢œ0÷Ä?Á$Ât?³7•%ÿä?¿âTR‰C¦?´óӅ5 ö?纴Å,úl?½	Á{A3FGL J1628.4-4546@uô!-w@kOÚ2æÝÀ8`É{ßtoÀ:aùӖª?ôxËéM!@ª˜zµ©@6 %#ü¿åî_ª¿é'*u°—¿ë9hÐ調îà#ñ÷©šUNASNone?µÍbíœ?´·ã/Cß°?Ôprð˜pD?Ìä¤ó«G_?ã$,ÛV%Š?Ï$±SԘÓ?½L<Cf?Â9q¸¢?Ö@¯F²?È#N'ËlM?á6 Üi™z?Ëï'jôXÓ?¾†	φp?§"¹*b¾?Ô¾²ÎÝ˗?¶7$èw
?áÏԗW)f?·÷Wª0˜t?±¯€•Óm?¢jÓW4§?ØNO‹`
?ºk•{Ë?á¢è'†?»U^ɪ†~3FGL J1628.7-8056@sm‡~äâmÀ5ŸVûW÷À9àÁ3;–¯À;'yLò÷Ú¿À¢XÕâ©@ÿ‡Š#@»ß"¥"¿àzò ­¿êððØg,+¿çúe:í<¿ïÿ€
HСUNASNone?îÜPâbË?¢©ÿñ¶o›?Œ‰Äÿ?–>µYBeL?–1UÝt%¦?š—y]Ú½Á?æ·7ê'?ÈãDpà}?ÃjG•/²?À 9)ʒp?Á¸ÙCðŒ!?º²"äƒõ?êbƒ\•?§a"-HGö?´W[lÝw?ž	{ÞK)¸?¸"Œª®zM?Ÿr6ò;Za?áš|™½Ú?¼Š¦"L$?ÂüºÂ#`‹?¶ÚÌ´®½ó?ÓMm¥ºÔ?¹«]œ#3FGL J1630.2-1052@ ¹™aÝ@8È!~|À9ºV4¿û-À;Y¦ùÔlÔ?òz(»
-@7î-ð~@a« §U?ïRÇ:f®5¿åIøopƒÔ¿å!'óˆß¿ïý…¿û‹°UNASNone?Ú q²#Y?Ì&Å¿Ý?à·>™Þ¿?͝šÙOÙ?¶ê<Dh|ž?¸fÈÔ@?¥ÙVÎcº?µÃ]0ûòT?íJ®ËYã?ºU+'Åç?¥{¼€GD?¨Ö˜·¤îæ?ܹ5i¸L¾?·ucÊ´J?ÙHÌZ?·É>—ÜÅ?č
…ÍË?¨õíhúlj?¥¿[DɪÜ?
Ì×ï?ê«Ô0#?¹ØXC0?¿Á°Üê{?´øvQÀ-½3FGL J1630.3-6126@tcGd­ÿ'À!Í_™Ã‹À8ÿXz™À;\l <K
?Í´#¼%hM@–)€Výh@I`p-:¿éÀGáɒ¿èTia¿æ¯tҏڿïÿϲUNASNone?ïî–QòÒð?m¶¶'óQë?;÷y\B}Ñ??—Y.õ>?[Õ}ÃI€Ù?lƒ+§˜Â¯?éEteµ1?Ʀpäñ—?¥ViÑ{'?§©8ÇwW-?ŕëº	LY?Âa8}Ï0ô?í¤WtX?ŸL"0Q!†?¢Í1¥û²W?"µþà^?¢í]h])?"
{k?ë×¾«ÏV?ªsh®8ñ²?œ‹…òÇ?–ŸŽ"aŠ?ºCÀ$ÏD?¨'.×Äè3FGL J1630.3-4346@u2SâÖ@	†×:ÇÀ9ˆ³c$"À:ˆpSO?ðrD˶ø$@
mœ@Ô@P`j£ã¿ëA2'^>¥¿æùdÌÍ…¿ë|[Ñjžã¿ÜœJ°jUNASNone?³þs€
"?µÇ?ÎN?ÅØHæ²q?ǟh¬d¾?è&M÷ãwR?ÌI½Ÿj?äÎ*±«ô?Ô¯š"xA ?<ژþá?®-d;@?Ԑ|ó,?ӏ:	éo•?Ó@üRpôÿ?°üS'Ýíi?υ"Ónš?³flz¶	©?Üüyã%S´?´V$^$†¼?ÑI»%…J?Ëù÷¢Bó?›zÒ!̆Z?¦^?$"%?æKÜjY)?Ì'9¢NŽ3FGL J1632.8+3838@NÞáG®{@EldE#öÀ9àõø?A^À;áý¶z?ð[(ã#%t@.£yè@žXߕ&m¿ï̦¨1@?çJ<M§í^¿åvzÊeX¿ïÿ—Ö²UNASNone?Ø9—Í?Í÷aZû‹ð?áU>Èl?ό'|½BZ?´qVK¢?¸þPÊõk?µé{YÚÛ?ÃÝ®þª8*?ì
QÇBU"?Åܟůÿ?£WìØ$ð˜?¨-X$L?à}BDããy?³îbÉ£Ÿ"?ÒZSÀÍw?±ý39½B?ÉVOjՃð?¬¯¯<' U?›y	¬bö? œ7§è/?îRZ¡$?­`ÁÎfE?š;¢/ÿ·?¡«ï}Œ3FGL J1635.3+4257@Pèñ€
|@E:ž¡@WÀ:O&ò³À;òøK֘(¿ò½Fâ½yô@-Yôèõ¢@U1\¼™¿êîÛü{Í¿àÏñ´&§x¿à$'rŒB!¿ïô'½ÌµUNASNone?ï¢Âþ")P?ˆÙêMäg?"sm‡ìIÇ?‡¥Ê_}ªP?Vޖ˜K ?ZîƦ<–5?ï tl?…Ï֕*å?wßýøå1?zCVH!ÿ<?wåúÆd‡?|ð{ÐÛ?íxSñ€Æ?¡^ÿpÆ5?«G¶S®?²Ü·Qn?šgvcA
´?‰•‹Ùz‡‡?凉»‰»j?®ÁÏ©D?Z{\xvH'?dº±è?«?ƒB%Ž'\%?~!ÂÜû,13FGL J1639.4-5146@tä
"M;À
ËšþôgÀ7ìú@£À:®ŽwýgŸ?ãÜzª@>`ÔV.
@ËBàO`¿àüöøoh¿äÏ>"¿äk°ã«á¿æÇ1'ý¦½UNASNone?áì#|xÑ?È#¥¿¥@?½ª3Ü#•×?º‹/%ºq?Ô½,Þç?Çaž4…™?У˦%z?ÌVp3[?Æ6d<\Y?½«ž^¨GÛ?⠁Ö,´?ʝ÷çQH[?ß@âkzŸ‹?ºV6¿dVw?À26Ég£
?§væóÙ?ئ/юò?·o+FÞÖ?Ø£®L$A¦?±á¤ôå?´––9kn«?¥<»2éo˜?áVÀqX?²à¿Ú¹e3FGL J1640.6-4917@uÕ<ÝÖà¿ýX™¤T(À8Y'£Ü»À:aÙïÊþ–?ìüÞ8¿_@A9ˆâ½$@tÿÑ¿äÞ~r
l¿ç~%q ù'¿ã0¥c@0¿é›XL-'DUNASNone?â7vecû?͈ñRқV?«·¾K?°l¹Ó]ñå?ØR™Q3Wà?̾8¥FÂÿ?քSâhQ?ѐëBÞ¿?¼Ò;©GŠé?½Nq{mx\?á#Ž™¢æ?Ðë,ˆ"-?Öº"#!gT?µp¡^;¤Ð?ÅUøûdŒ?«öªu|Ÿ?ޚá_Uff?µí(È	?×֞hæûF?À7êU†j?ŸòñßlÊ)?'2Ôebêh?ã<'?¿Ð"¶$ʹ3FGL J1641.5-2856@uü«¾Ê«Š@&ÄÝÛ
À9™­»ŽÀ;6Õü÷7?먕_ùõ@tî¹[¬@] A"ô¿âH`q"Ó¿æ´æB®j%¿ëU¿]´¢E¿ÜhW΄C,UNASNone?êqqùVÆË?¿'ºÇ¥
?¶ºõä®ìf?´§)…Ìh?µ¹zPšÝ=?µdpšìþT?í/:P'Ú?»t#9Çtï?••HՔòf?¢ÇèÒl?± ÛF
""?¶
¿¿Ôä?ê͉-/ð%?©ÿŸ¤éW¤?®6|óÉ-Ë?™EÛx\Tb?ºxx›çö?£Ή±µå?çvj$ge?¹RÅ+[€ž?°G4dzr?°Ÿâ¢bò?ʽ
Šf1?µ¼Œv9ºÞ3FGL J1642.4+8045@\oÁ½¥@?ÁP¹U÷ƒÀ:A)Ý:ÙÀ<u^Pî/?ÜíÔ¤v[@j×9bL@áz AÙ¿ÞÎÕù#ö¿åÐ×b¿é÷Ös¿åSCTF0ïUNASNone?ï!'â@ó=?¨j#äØ#~?"Ù™y‰R?§'ßÈÁ?€Ô|°ýÐ?…~6¡—3U?vrj?£¥h\e	?š0{oçº?›+E'tÊ?'«*ç?"ÏEÿÚ?íŒÁÓvVÙ?ŸAæC[·? ð#§ˆî<?•¶ò'ÍPŽ?¦C¿!¤1?'[0ݝB?ìKåãG²¬?¬¡Ü'ÌmE?±™mtæpX?¥2R…øÆ?¨Æá·ô‰?¢'Ü>²h
3FGL J1644.4+2632@G;Ž!–R½@C@oiDg8À:*=h@[:À;¯³æKùÔ?Þr[…?x@
÷û%$ҝ@–ˆÌB¿èmsZ›Z¿î¡·ú~a?Ò½š¡Ä4¿ê,9ÓÐUNASNone?ïµEé?¢I›=-½?jï§S¢u? )8û(@Ú?x‰Ìü$¬?Çx©ß?îÝYÊ&R¬?¨øÏq^3?–àürdºi?¤Æ:â9?Šç"'¡à%?'É=Í ]B?íœ×¨$¤Å?ž Ñ¸áX?šDèÊ?Œ»1Ë:É?©"‰ª°I?–Ð!gï?í•ÎŠßÉs?²;)Œ†½Š?}¸ª:wd?'%7ˆwºÄ?±ð^ó?±uò'HG
3FGL J1644.6-0911@!ZWɱh@6ßpyåŸ,À9¢{…²\À;5£"ŸY¿ÕÑÝHו@
5ré×u@‹³ŸÕý¿äÈ^gƒ5Ä¿ì{"'È¿Úqì"õÆ¿Ùp9Ðþ'UNASNone?î$öŽy—ý?²âÃf"L?hT(Cäá?nZÑþÚ´ß?¬+T"(>÷?²b¡w?ï¤p$	`?K'ÚC6¿?róñã•a?Þ}»û>?zÔPº–?"¶Ó¾"á?ì;aà况?§§;遗?—ÆT§td?‡4žß®6Ã?¸aÿcXÕ_?¥Yïá2_V?ì¹½îL]?¥½f©$G?TÆ3ÊÞ?XÓlEÇ*?¹á¥tαð?¥®Î‡j¸3FGL J1646.9-1332@ÏV!tÄÎ@3ä_ö"FÀ9ý»´v"²À;R]¤öÄî¿ó²¼ökÕ@
äË+­-?ý›ÃNúº¿îå±ç‡ýÕ?ÜŸŽ%G7¿áJé&¿Õä£ÖçáYUNASNone?ïÞÑÒb'?pñ0"S$R?Lf2í?M½¤[Y?j¹¢<!?m¸	ôUîÖ?ïÇÉ+ªí×?aG.÷È­?c­ÉWa;?ké̂€î/?rD…ãÃ?x'ƒ?—?îÔÍç,'¼?Ë2óªu?ˆB‰ëÅ}%?{ ñ?Uµµ?™Dþ$˜Iî?‰(´$
ù?ï"LYªèÍ?…¸6}:Ì'?<£	[q#¸?Bòç[9Ó?ŠÑJjC±?…Œúªh"{3FGL J1648.0+4230@PÄ:}ªOÊ@D÷œ"/¥À:kªKÀ;òÛé B*¿Ô\È/%©Õ@|s(@»Ý@×mŠNοàC±‰`¢"¿éæï'7ñ¿âŠ
î¥H¿ïç»ÊŠÁÿUNASNone?ïÓYfóã?yÒS[´^?U_ï¶.u:?W-½,
€?pû^úqL?v†—ÄO?ï~i8á?—"ݹ ÷?#õ•§K?Ž™ž*°nÄ?‰z†©Ï?‹Ò™Y¨uS?î#ñ¥Jç)?—jpÉ×?œE_²³Û?‹À77áM?Ÿ<k£ïüø?=·AQ1?î¡{†ÎÞy?–ã—×.€	?‡ޜ¯Þ?'1ë
‹š¼? %B[jìx?'é}NÎ^3FGL J1648.6-5635@t·k¤"ÈŸÀùõß덂À9CCÁð`À:ýàl¼Á½?ôSÈ)$@
)œ–¤Ô@hž\‹¿ãžõ"YŸ¿î‡Ú%—¿äJÅk¿ÐŠÙD¶UNASNone?Ëû$æÏs?Çê³ßÐO?¥E²öïå?ªãæS"I?ç¬ÛȤ½%?Ê\¨ó?㖲´»ßâ?ÑygÅÿt[?°ãÊ2ÈÚX?´^«UÊÒ?ԙ¨	Ö	¤?Íwsç|»P?âBÉ=¸
?³2óóD"?Âæ¯×h°V?¦ô;="¼?ÒZ"Ð7Á?±S×aó-?à°J«ÌÛ?Ä.²C	•Ü?±¼ziHJ?¹R˜Á s!?Ú0LDVSË?ÞläÆù3FGL J1649.6-3007@vð¹@"Šl~®[ÈÀ9
д¸ÙÑÀ;!Š{¥?òEaƒ¨–@¸¦Í^Ã@"É﷿ߟ-ý¿3¿äõ힇¿â˜µ˜þ"¿ïÿôo±œMUNASNone?ÖÉ áã…?É°P—Ì?Õ³­|ü¯v?É
>ϓ#~?Ӄ1¡ôm?Éab×?ÐÒ'yi/?ÅñÊR Hh?Ú-U*²þ?ÆxhÒL¡?Õƒ[ãìÍ?È÷9ñn?ÛfÓ}+Z?¶--Œ þ¬?בEyÄöJ?µزµ?ÊÎò¹?«ÜbÄü?À?ÕعÈq?²Þ"*lՉ?×6¡lJ?»>
?Òð¥tàí|?´…pá3FGL J1650.0-4438c@uMIº^¿–ˆë¡y6ùÀ7P+ÃÓ)À:
™Îr¿:¿´ñ{Nr,W@Lóin¯@«"¬î‹¿åU5_™~Ó¿ç²¹'[ÿ¿å™»µÎ- ¿ë	—B¯0UNASNone$?®Fj@ãÓ?¯úä»WŒ-?¼5S±tf¤?½é´r,8?ê"ô-dï?¾O/€ïE?Œé½Áß­?¡Î#΢?³€ÜίK]?·¯Jƒ|ƒí?í=o"š9?º-aÕéƒ?ÁÉûeÂu?¨Ý®®äí-?Ìýô§2 Ù?±ÀÞ®¡×?ä€WYç,?µGyMÿ?ÇÊÊÅH?ºv 5áa?Ÿú4»J!?ŸWšÛcµ/?é
|ÏhӋ?½¾x‰ƒ3FGL J1650.0+0356@5Û;BÌ-k@<®ð®SeÀ:)CæÝõÀ;•ÙÔóü¿ÕøD¸0@[ÛB±Ux@S€?ÖY¾¿é¹€á¿â6 $š‹~¿Ý["¾¿ÖLn£UNASNone?ïð^kTr?£e¢žfĬ?Mª  ÏRö?–*}0¨?PmÙF´/?›cc3î²&?ïЇT7.?y‰À¡°?bÐÁç ©?f§£Ó€FÍ?l§ê®ê@i?r–òðÐ?ûÓ¬¦?z¨1‹å?pG[¨>.?ho§
ÜÝû?€0S|À·Š?uÂ#Ö"iA?ïÑŠÜ÷R?ntå…`³Ã?kI€ÎY'?¤P)î?w3cþ'ºÄ?nE"äӍ3FGL J1651.5-4626@u9²þÅm]¿ö~'MKãÀ8ÿÔqܼÀ:2¯È¿ÿÛÂMíɝ@
dy¤†²Œ?þ¿+ie?ç"LšÀÇ¿ãi‹™Ì<¿àŒŒ¾¿Ä¿ãì·£2UNASNone?+€Æĕh?ƒƒ±'ÍIn?pCŠ§¿?Íh™x½/?ïšËƱØZ?"«¼Œ?Ý¡ºÀ¢z?×âÕqœ?'ùÞâ+?¡°ññϕ?àž'×/Ëî?׈¶Q®Ì?Ƥ}ÜÝ55?«‡D[¾—E?±œ2]©˜A?ž֜G·:?è#Z=ª?¯tŠé̇g?á×îË¿Ož?Íìô̒ÕY?&\›™°	3?5Ù[Jãè]?ÜMVÕ*Ã?Íík!z¬3FGL J1652.2-4649@u5ö_Ø­¬¿ûàÛwŠ{À8¹°,À:=yaë­c?™g¾yNªÆ@ët±­·‰@»ÍŸ°‰ö¿êí\Ò
q¿æÝËu'[ë¿Ö‰óü3B¿ãክ~ºUNASNone?Ö»¾xïÛ²?ÊáK‡ú/y?"¾s²È1?Ÿ%¦'uã ?ãü-%÷Cå?˖uå``ê?ØAÖ¥J?ÔQŠ·2?¦ø´R*ù?®«
?â'ωhQ,?ÓèxD<·š?Ò«´.µ?³éÞQï¬?ÀÑrøóY¹?®Öztõûw?âuÉ*h¦R?µ"?ö¶Ý?áÀI‹H*â?ÈÑiˆÈÙ!?ShKµ+ä??U×Í@à?Ülº~W?ÈÏ´îaƒ3FGL J1654.0-4617@u?ž£Y5ü¿ùҌDF€îÀ8Ձ×ÛôˆÀ:a6=©®»?íÖ¯Ÿ?uâ@[ã‹U38@Ÿø-y?åÅ°óADˆ¿è6
g¾øp?Öñ\Û¿âSY<÷UNASNone?ËhLaNð?ÆYŠ?…¸® óΖ?‰€¢(†}?èâƒ4cÝ
?ÆV˾°{æ?ɦyw­%w?ÍÒÂ72g?«B»á2ä$?® N⤎}?çâ5äˆ`?Î}¸c¢ÍF?ў®À¾W×?·ŠËô—ø?±À™"ÙÑ?œØ7*ô?äø•~Ð8Ú?¹H-ŒO1!?Ú§á­è?ÇJC¹âàN?zx0…"'z?†©']Šp?âw'®X¼?ÇuO5ªº#3FGL J1655.1-4644@u<`ÔV.ÀO¼ä!}(À9GeÆ-vÀ:jÏЍK­¿ö'kØ@
«Ñ?þäw¡!MX?ïýt&Ù?¼ú]‹˜ÇY¿ìDñ/
¿Í)ȃðnUNASNone?ӐŽÙF?Ì=ç`¼l?´™îË »?¶ž%\Ɇ ?ãè¶ÞT{ü?ÎyòFÞ=	?䰂÷	‡ù?Ö¡ž-Í?'¨©¸ê%?¥ºx±-K?Õto€aj?ÕùË0)Ì?՟Ïr¤?i?´i›4s?ÀÎù«Ó¼?¦÷
´YÀu?àüYÛ¹\?µÐÆÒ+3-?ê݄Þ¿?ÁOÆ&höà?bœ¨ÉÙy?x|½ºðM¸?ǦL˜EŸ?ÁCdëu3FGL J1655.5-4748@u/€IQƒÀ1Ÿ<pɗÀ9	ñ}†=œÀ:v¦ ™@¿÷ú­¥ë§@'6µð@ü½¿h¶"¿äBVãVž¿ë}»Áãe¿çìѓ'¿Ñfn`¨-ÓUNASNone?ÄÎÔäT¦?Âc‰Tèõ?ð³':E5?—šñ%^àÙ?ês†®µ¬?Ãy·ä-É?çdíÖ
I¸?Ѫ§Å0ð1?'øT~ÿ?¡­±q>è?Тþ£Œ€?Ñy2¸–Ü?ÓAœ‹Ê²
?¶¹)é¿ÊÖ?ÀĚ³;ï?¨€ù‰Ä?â.
Kæ½?¹.ÛÍh™?ê©?Ž[Ñ×?¾¡å‡ÑlÜ?*^É[ð?"tî?­e?ÅX¡Dßw?¾¡
¹}÷3FGL J1655.7-4712@u7P›ùÆ*Àhñ[!ŽÆÀ8ìùTëàÀ:O7iù˜Þ?ã·Ñ$m@
ñk?¦@ൟ´Á?ïÿÂ8&ì¿êú(­Âý¿É
~XJ™×¿ècÃ`\UNASNone?Á"¢Ò÷R¥?ÄÞêð|s?¥ð^''¯?±Aól=îÜ?ê<b*f?ÇÉZcY?ÓÕþ$k¸X?ÑÕMM­ƒö?µB£'À˜h?¶s/‰z«ô?ãl¬ˆÒÇ?Ñe¿hð?ÏÚsÆU?²µ›H*uÖ?º¥¬®eT?¤;«Yˆ•%?ä´­§Ø­Á?´L
â{×?ÎwöÈ_ì?ÂÙ浍?Š	ؐ*úL?h9$ìô?çùÚ많?Ãp7.?3FGL J1656.9-3919c@u›ñ©ûçm@«€>~ÀÐÀ8ÙZo¸ÀÀ9o+-«3ö?îuƒ2Wž«@
pµÕduö@ŸÁàŠ™Ì¿ìzÛd%¨¿ä>lbm¢¿â~­®Ñ¿é¶Z'àùUNASNone)?š³WP#"+?¤™8H"‹?Ó¹—'Šû?ѲµÙþW?åM™|¹f^?ÒdËÎ; ?âF$»‰˜?ÕàS¤›+?¬«Le IW?µÄî«'?×ÞLü8ÆÌ?Ô>eÅa2!?ÉåQ·~«h?¯sf"?Îz®þƒÑ?²lâ6yiÊ?áè ´1?´l¡®t·›?ºC \ñ¬¨?Ã1†*ÿ$u?"¨³?åÎJ?šLú$J?ìVZb›ù?Ä{´{ÊäJ3FGL J1657.6-4653@u>tSŽóMÀÙï_žÌ	À9à>™˜ÃÀ:zBf¬ÝC?Ò©BeøyÆ@!ЂŽæ@i=@}H«¿íޛ›^?ïý°X瑎¿ã¯ÉÈ4¿à"‹Y"‰UNASNone?薎ˆf¶?ŒìˆóÄ?O¾äW"?Ïù˒h?ËÐÉñHóî?Åc¾cøp?æàt"áI?ÒyÔHïm?§1Â}Èì?´WÛÒY†?α½6?Ý?Ðq±zy¡­?ەèⳓD?·øõ mŽC?¼c¼%?§R§J"Tþ?ÝQ'ú	j³?·]3Í@òÀ?é.äÚ­?ÁÔý²öG?¬½ŽÖçÓs?¬t<û<?ÄŒ¶ÛW	?ÀPù"ž°¥3FGL J1659.0-0142@1¥Åo@7èSŸºEÀ9E¦N³Â:À;9ÏÆl`?ç2ˆ?¡x@$'RxGå@Ž™`cÂó¿Ùœ{©Í!¿ä𫲱ÿ¨¿Úþ£ûXŒš¿ëÃy¸sUNASNone?íË$ùÙά?°K¸ŸÙ6?£Ï¢P˜>?¤¸'.Eœ?žü¤$ùì?¤§vLN?î*ÿ<*¨j?¢Æ@Öƒ?¡ìžp¢qH?—1R¡q¿Í?–Æۙf?˜nU>ÿTI?è¥nd"`°?±"·"Ñ,?ÂZŠ'ÅP?«–fß'n©?¶xŒRËÛ?¢à´hŒs¡?è¼Å?ª6ü،ú?¬#ÉW~ö?&[XT¨,?ȎÁŸ-;?¨/4òõ°83FGL J1700.4-4019c@u•ê~ùÛ#?ó/ˆƒÇ À82NÛËÀ8—"€ãÀ?òw"pèu@Ò]×K«Ð@'¯ŸëBY¿áÔ.LæÚâ¿Ü|ùÁm¿ëå¥:%"Ž¿å&"g3HŠUNASNone$?yÔEH¢ŽP?"qÞEM?ÙKpZ‰s?ÔÖS@à
?ã&ŸHav+?Ôߧâ&Ҕ?âolq^×?×*R¡7»?²Fq»±<<?¿SD}?֏‹Ž0óD?Õ¨ŸS\î?¼ke³›X?¥9\Ÿn1?ÑýÛ¼#Cž?´}²Aµ?ãs¥kzú†?´ŒP®è2·?¯Yç‰N+?¿Ì)`‹?Œ±ë(HJâ?—0I]1D»?헦äæIò?ÀúlÈ)£3FGL J1701.1-4930@u# ¥&•–À42ðîÀ9peÓÀ:«Wãä?퇩Þúæ@'$«@'ÛŸx€Å?¿hf±9ôC¿ì+4>ԅ¿èóO™'¿ÌŒ–"w8UNASNone?Ø»Q¸yæx?ÊÁ"ÖZ?ÂÃAV™÷M?Á™*9Wì?Ýã
œ9á?ϱˆ2Ï?âúüS·û¾?ÒM}; q•?§PÊ\?'?¬S®£Kwf?×î

à?ÐÎ5^⵨?ÙhÜ÷†B?ºfÊ 9L?Ãr1u¼Œ?®d4Ä]Ì?Ý2~h*3·?º­H/rG?áq=!ƒÒ?Ã5ü•4?–Ht0·~?ŸqÓ†?Û¹•µP_?ÃÜW¤3FGL J1701.3-5216@ublvKÀüÂ]ÞÀ9‹i"ÙHÜÀ:öÔ2ò›"¿æzB÷ÔëÞ@4Èaƒ(@Ó«@`m¿á|_)¹À¿é|Ρ}¢¿ë—¨ÁæÐë¿Ïß:sCoUNASNone?æñ#cÃG®?È
<^è(?š§[õ°º¡?ŸÆя"?ÐsCydú?Çpgÿ²EŸ?îRQÖǀ?±w$ tbå?y»! ý‰?0Hw³‡é?§£~_hM?­Éäh‹ÆH?å¦×Úbw>?¶pV´Ï¶'?¶03ëBÑô?¥kLҍM¤?ÎL† Ôº?³m§Ûåí?ë«[F¡'Q?³SI:XÍ?P'2rׄ?Z˜5X•T`?Á1Ž€"´?³IòQ¿®»3FGL J1701.4-4654@uD¶°_¯À÷d»k{yÀ8M·Ñ"+À9ò™°?ÎL?ñˎ6.í@Žà®.@àyQû¿ßwB(æË¿ê¾þ¬Ý‡õ¿æ¢	sWvÆ¿ì¯2ՀiUNASNone?&Vê"â‹?'\ù"·ª?À¨9_- þ?Á^cèù3%?ëT¾ðàp¬?Â/²Ç­{?ÆOüÄRpð?ȇ"¼Ï\?ÐGš7òÄ.?Ä£ípaŠ$?âH3²ò­?ËBf†ü?µÕ`LAÑo? üv¾g'1?ÑùdyRü?³¦(ß|j?äHËÄ;T?´¾ÜÃI?²—<ÙBL`?°/"ˆk?µûåø"÷?¨}Õ`
¿?ê훥Ç5´?·ÿ@ºÙ¼3FGL J1702.0-5414@tçõ£KÜÀ"VÿÁßÀ9°—  À;-X'ßB?í,ýÜÂÂ@𽢍^@ càz(»¿Û}ƣפܿéʓõÉMð¿ë]b¢E¿æÑÑ䎵eUNASNone?ädHÆ`ä¾?ʗ{ÈTÀv?§±ñ…MU?©¾Í<'?ÔA0BŒŒÙ?ʚêZÖè×?䑅žs¶°?Î-9ê™?³+!÷ˆi?³€À÷u¨?Òiúš°ƒ?ÈA™¤ç«?æà­Ì‰`ƒ?²ñ,o2?¹PV®›ƒê?£úŠ~ýqë?ÇÕvŒ»þ?­4Íg¹?މÁ…?º£ÁKuÿ?À Ã66?µ:´»g?ÙfVÜ#2?¸"F4'Ú3FGL J1702.1-2524@vWñ6;%@#÷Úè'®À:>4ð¢"ëÀ;_$Ÿòy/À
tq£~@	ºˆ\Zsê?ü&C@qŠ1¿ï§Í:Ÿ§ê?äiáp¦cà¿æaW1rÇ?ÈÕ%‹Õ·UNASNone?ïíëºß6?¡HÖQèÛ?SbˆZÚ¢Ù?YãâlŽãw?yPhÙ¼1?¡8Xõ'¿?îÆ[ŠYëm?²ÈF,‰?n§—M
?›Ϙ-=–?¡¯ÕÐìxs?±¥:´|g?íúù c" ?—Ýh˜!x?"œàÐÀ·?"!c;Py`?¦ý'fZ?"·%¯ê'?ïß«þۛ?xBƒ™êá>ç­ù—j?6Êåýʶ?pdS±&?x@eЩ³3FGL J1702.1-4623@uLw[0À,Ò@ª;À8™Éõ÷¼À: 2:ð?ÑOš+(¼|@Xî>Œ'°@Cà) ã¿êÀ`*76"¿çèáçwY¿éG»¼•XS¿éÀNº«À–UNASNone?Â."<?¼	@&Ô?ȃyPŽ´?Æíl9Ê£~?åS–|éÕ?Ëö>k-à?áù|{Ü:Ÿ?ÓRý¡l•ƒ?¯"W?³IOÀ"µl?Ø+‰TØ8?Ñ|wy0¨?ÎWðMÚLx?°y\eC?Îõ§"ªÚž?²lIZw?ଚ^¶;?µôŸý?Ò&h¡ËOÉ?ƎÓœ
?†øôBí?~ÇÂÐÛ[µ?æë«IN?ƧèßÚ§ü3FGL J1703.6-2850@v.¿œb¡¶@™?¯BxKÀ9Úæùž¼ïÀ;1ç£è§õ?ÔîÒ¦U"²@
T£ºM@ЕÀœï¿è¬RV9¬¿ß‹^žµ§¿Ýhm¼	õ¼¿è1[âÔËõUNASNone?뀂dÑ°ü?Árï:Û?š0ÈͲ—? õ$³Ö"€?½z`§?~?ÀMêó<Ž·?ä\þ'\ ?̪(XÎü.?¾_¨Az?¼´2Ÿ"§?Ï=Uâo.Å?Çg`Íèœh?ëiã‹pB?ª‡ƒÒÒhÒ?¤sÃp¤#?'¡'Uq‹?ºwì+äT?¥Žšr•w¯?ßj €Šã9?¿Àæ'Š9'?»¦² I¥¿?°ÖíÚ5bº?Ù¬2×b³V?¿ø×!3FGL J1703.9-4843@u1³:}ªÀ¾ «†+À8ÀUM9n·À:¦ƒɕá?ôƒŒçÚoM@
ÉfÅ=@àVŸsù!¿æð¼ÍóŠÉ¿á€Knµ·ª¿ëMkÙ xd¿ïðÊã
]UNASNone?ÿ¤ÈüU?‡ž¦õ·Î?êÌméÉ}Õ?ÆøÔ7­?îV¾xæ?Ƥ›•Ðœ?Šc€Í×y?š)_ï"Ã<?äz1—ƶH?Æþj]ƒ?Ö8€Ôl$µ?Æ%;]?½Zë»e"3?¤ßa
aò9?à/ÚY°€½?´óäDøÑd?ØI]ŝx?µeøïHÉ?©ó–Ÿ?™«Ø9'¬Á?äÿY&¤å?¼˜¢¾KFY?Òݏ?ô]¢?ºÕû–v233FGL J1704.1+1234@@;‡½Ï@=l§qÉpøÀ9d¼¯HWˆÀ;|ƒ-±¿ç¬LT'£@Í,݃©B@ªŠÿwïÑ¿çÌBºÔk–¿è᫦·d[¿ã5àçX`·¿âùs–G!UNASNone?ï`¦tv9‹?¢Yå†?Ñ?]=t
Þ$¨?†@8ÔÈó?'Z0ŠìD? ièìê¶?ï¥1xC›Ï?ˆ=¨‹&|?s۞Aœ¾ò?xèÚ\*?y‹¥œ•Y¸?€1½êa?î
V˜[Í?›s÷ûíMP?ÙU©¯F¾?€¶Ñ©Æå??¦â¯Á¢ŸÓ?–¼3a'2g?_AŽ·?•EnHxY?X®E\ú;'?X¯(օêÑ?¥¡àÿBª?•­EK3FGL J1704.4-0528@-Óp&É@4̽±¦×À9Q!Ð4`ZÀ;1°(QWá¿ðG˜7™ÊA@
ÖHtÄù@zZ Šy–¿·pCR…Ëì¿êW1zKuŸ¿ËdöU¼¿åù…µê¶UNASNone?í§ù]¡?·+¦{iæ?yB/㛸?{ñ&ä%a?±,ÉEø?¶ž­dCKR?ïŠ!7Pgw?–@âqõî?rMc gœ?tÛP1ú¬?"Q›ÝîV?"v3rø=ë?ëo¬P2?«´Â8õd?£55A Ù?'YLƒ¢I?ºù/Oü®?§úgc¸f?ìatŽ!þ?«©&ÒH*t?HçÃQÒv5?P½$–£#¬?¼ÂŒT+#?«›É'Šg3FGL J1705.5+0948@=ÃRü&V¬@;ó~€8Ÿ"À9¤œ«fKÀ;v¬Ö(–?⠝^då@žæ$a´@sï< ¿äËߏG0@¿ëº'fZ¹¿éØ/_Ìî¿ïþ±Ü[‹UNASNone?ïE'ªç?–÷YÐ \?…o–#H?'Ú[Á³òé?'ßÌ߶qi?'á°^·ç?é¦
†ë,Ä?»~[ËñÎÁ?ÃKÈ«û9?¶ˆ12xä¾?¨pJFì?§úµáö7?잺'¾?¢xPNUzÅ?¨>éZ¨½Ð?'•êÝÈØ?­Õm"[aµ?™NTìÃ-,?ßJ(ƒ?µ¿/7éK?ԋá¿KÀ?¸‡Ó(Ì?ÈSì`bSí?±]éj& 3FGL J1705.5-4128c@uÕϪ͟¿Ñük`v7jÀ8A[ñ˜^0À9?m?ﲕ:õ@{õ¬"óí@#9ßÊ«_¿çrèf›‰¿êãýVb¿àÙ¯Ü|S¿çÖ·p³áUNASNone)?•fyÜ`<?¤FVÛ±Ê?µä½œo??ĸLåï(?ì˜4"½?Æ_Í­}ÄÅ?ÇF}µƚ?ÎNgHS—?Ív'ÒÃç?É1G)!?åKò
`?Ò2¤'$X4?À§q/,ØÜ?¨ƒ}+øÀ?ÅY-j˜Ï£?¯\jA_å£?æØYŽ•à?²‰S	oŸµ?±xYàd5r?¿­	:ŒžI?~žè½Z•S?ŠÚ)"âì±?퓶òxÄ'?À'÷C¡"æ3FGL J1707.8+5626@U-þ®û+@B@­ÿ'+¿À:THùn‡À<«ƒ¦é
?ÐA(J29t@
±[UçH@
¨_°Ù¿íÞ¸1+¾l¿Ô}À³l‡¿åY
^¨Ä¿êJØ3ÙµUNASNone?î•E²?­æám]ñ?¥Ð23µ‰?­'%<M¡_?[ϯ\Ãxb?e´."p™0?âÜ©æ3Ç?Ï1¸âÖú¾?ÖA‡•ƒ§?ÍS]çwâ?°'xXý‹?®L­kœ$?ìLÜáf½?¥nLïÒ?±eo0"ÎV?¡¦(înè¤?¨gSˆŠ'ß?".éreÌ?à·£#:2Å?ÂË,9'êV?ÚÉ{1³0o?ì	bõ"?®9ô>ÃPF?¤Wµqß
R3FGL J1709.4-0917@(d ]Øù+@1¹‹Å›€$À9ZtŠìW­À;"Øzøß?òŸDFx@L'Ûç@·Ðß´0¿à°2x*è¿ää0ÌÚj¿ï¡a+5…??ÜH¿,âGoUNASNone?èjåò&þi?ÇV,{;?Åp¨õ?Â1YKå"`?²ˆv"ž?¶.è÷º?ïgGít–C?¨%E÷¾?úCÁb+´?¢$kºm?†0âÂ)Y™?™ ¶}ݤ,?çq°-צ?®m©«*?À庌«P'?¥­§+}¤?ÁV>²Pã?¤ˆóo6Nc?끹R&äš?½ýdn4J?¡a3mŠc?³ ²ì ×-?»gÕ?¸Q5J-_>3FGL J1709.5-0335@1Uœàuöý@4²‰üm¤HÀ9\åüH»[À;*½é§Ï¿Ùijû@&ë$üŽ±@Âb€}¾È¿ç;£g ¿éT_0o½¿à§mƒÕÑÈ¿ïýåғqsUNASNone?ï+dC)?~? M¹äž§u?qð8âbs?vüw+t?–ib?st?žœ~2}g?ïæn¿ôš?›-M}& ?'Ùjªi)?Š«™Õ֌»?óŠåXpl?"§•g¼?ë'ޘ¢?©7ÁóË*"?¯Õ¸ePDf?›äÌ
«?´äؓо?¡ÙÂÅ¥õ†?é"±ä?°ÌtĂ&?'ÑmkøsP?V%Õç̎?ÇyÆ/¼î?°]mjE²›3FGL J1709.9+4624@R÷´·@B1C¿rq7À:\ìOIoÀ;ðö'9)í¿ñ>ÜÔ׳0@
öÑÁŸ}@í ,ì¿äì>
ì[ø¿éÊñ"žÞ¿ÜI˜Ol¤Ä¿èA»püUNASNone?ﭓ-om?"ÒF$F‡?Ps_$ö§™?YýHº¦'?'ŒÈ¿™Ïà?">Ê­•Ð"?nmÁ?‰ûF‡gn?vžYÐlf?|¥y<?zá[x®³?€"k~uD?îC ú"L?"çì[,O?ÔXÀ`NÇ?€ž«èþ?¤Z§ÀEǂ?':XÏÂE?ïo6â%xÛ?†\!¦G?GÝ#@·Q?Iîaar?'Z:¡K(»?…Úˆ2©\3FGL J1710.6-4317@u'•éᰊÀãâ;ëiÀ8£bþÒÙVÀ:3T9¿ç+"Ÿ¸I@i›Â"¸Ú@6¤€}há?ïÞIρÝæ¿ê×{»Ñ싿奡mV"¿ç"§4•fUNASNone?¿KÑÃÌ¢ ?¾ª[ÂYÖ?ŸWøu2>F?¦Èû¥	¢?ëÆÜÙº?Áq7»‹²—?á¼Áƒ/R?ÔÚ
ceîÐ?¡þyøFžÛ?ªöeŽW}"?Û²·=ð́?Ô¢óU?ÇåÓ}¨'q?¯t±Å]Y?À;¦ÖGˆ?¨v™}?å÷ÊvàdB?´ÆdÖ?×
²@ˆð?Ť!†_?oqšóáH?qãg1›÷?äYµÉ "?Ÿµ~±3FGL J1714.6-3327@v	9-Œ*@Q]À¥wÀ8ãÀÏhˆ€À:u¡¥×•~?èXç³ê@Ú_c<æ:@ۙ wï¦?ïû7»'U¿é¤f"a¿Î'èÉ
S¿íyü‰ÐyUNASNone?Òûà»{…?ÌËÁ©ÅÙ?µ.ÌC,?¸˜•-p`c?ãßiÐ(éX?Ðg5œ>?ÛI<·<²5?Ôó¤˜yBù?´mzCÅ?ºØ|IÑ¡?ߛd·ß'?Ó¶–¨:8?Ïãªuga¶?²©à­óvå?Ⱦó?°PqhtF‰?áאžêÍ?·!N?DÝ?Ó¼æٟ?›ûå$%Þ?¢ÔD;μ&?¥¬6ø<?åR]HÖD»?Ä·–5÷3FGL J1715.4-4028@u¯vݬîá¿òÇAÝðáÀ8çw ÈÍdÀ:qΣf¡ö?Ô©{¨±©@^9ókÇú@ÕYŸ®†'¿ïٙ{‰Ã?äæBÙ泿¯ƒû¿û¿á°ŽJ'ÛUNASNone?ëí…3ø?ÁèG.B?€Îl·*×?ƒ—狧}3?Âsc¿V—?Áª! T¡ú?à¾Y°ú~<?Õ§pÝ[&"?¬ÏeGeü?¸D[[Iv!?Úé_õ`)?Ôf®¥Å&Ù?Üçß
îŽ?¸¶¿Ûâa"?¶©F€ÂÜ´?¤¦ÃљÂ?ÝmÏXÁZF?¸2()V?êÓßS˜?ÀÂËA[É?xþDêù?y"Š¥?Ãï" ŠJ?À¯KDø&¨3FGL J1717.6-4404@u"^Ñ·ÀÌ2ùQÀ8nzj)i†À:n½º
Ri?ájÜÄÞä@›N•dUÀ@s¿ÀIÝ¿å \ÂVYÜ¿èl¬yxÅl¿ëºˆ×çC¿ãšá?S0UNASNone?ßfÓwÁÿ?Ê%(÷0±J?»üm'Åë9?»Žx÷0æ?ٚ#Œ†?ˍYJ_Õ`?Ûx¹±.?ÒÇϣť?¸©ñDú?¶Jî#ÝS»?ކCdUÁ?ÐÌZühëV?҆Çã˜?¶™ÀÀ'#?ÌoË@'H)?¶Ø8r 
¤?ßAR|ÅÛ?º§€8Ù¦?ÔÛ¡à=†o?¼`ž¡/v?¨!4ú]¸?¢ãܔÑrG?ä	<ü'–î?¼ºìγ3FGL J1719.2-2433?ß&•á(N~@E#ŸAyGÀ9Øïþ¯À:ëьO.;¿ê{—Ùƒ@
ti?´¡@QÓøÿ¿é®z'/Î,¿ëlîïr¥J¿Ó‰Û
àÆÝ¿éu;ss•#UNASNone	?ãUþ`b)?ТJéb?ƒ€Ò2®?‡}sc]M(?ظAb'?ÏáæZ?ëW—ñr˜?ÃRå;"̔?ˆ{æÍèPô?Ž¬}
QMÍ?ÁáÍW ?ÂuN`X®k?ãaìeýT‰?·ˆDìfq?²H0Æ;ÍP?ž¡KO"?Ôªvc˜?µ‡ø™–Îí?èƒCû,»'?»)oü¶×?a2ã"¿i?c·-9¶±?Í®ÃGÀ†º?»/\ÍÚ3FGL J1720.3-0428@1þ}ÔA5@1ìaAcwŸÀ9àÎÏÜKÆÀ;1s?'½À6·$ÄÛ@á=1¹¶p@°§ÀMãc¿åq3†6²¼¿ëØq›Dœ¿ÝèL@[ ÷¿Ï0Ÿ\H¢©UNASNone?ïj
&žSÙ? fɓd2?1n¾Š½O?=íãòïf?'zq;Yø? QÛÈ
ÚL?ï•ÅA£!š?wû
Œ¾?_7T'ܽŠ?kýß
?†§Å<ï?›¡ÿÁDÀ?íŦ'È«ð?¡ü0Fø5?‡ù<­ñb?ƒƒã#óÿ?­§Q"IĞ? £ú=÷ï?ïÂH‰bh©?~T•dÀ	>¡+ýŠg°÷>¹±­ª^s?~Û1îßX4?~âÐb3FGL J1720.7+0711@<ÿAJM+,@7i㸡œÀ96BhZ\mÀ;MbXº¬9?Þ9ëÜåý(@IŽ"«@Ï€oÑõ¿ãý>QŽ,¿ãgnöÐ"å¿æV	–¤=¿çãr3WŠUNASNone?çZ῾§?Ã昢Êæ¥?Á¡Ê÷?»·?Î^å<?Áy×6ðU?½ƒ;Aú}W?ìˆLäåÿ£?¶®ë¤ï?²…¬È/?¯åY-¦\î?¢p†Fuq?¥¹Í¿2y?ëxΌž!q?§õ•W;ø?ªä7¯Ï'³?–!Uºã$E?¶ÇoÃ'3?¡æ<†x2¶?ã«R·$ß{?°~N&'R?ÃG<Ùk¨?®«ÌBzƒ?Îy"h?­_}€e3FGL J1721.4-5253@u·AJM+À"4!ž¶9
À9Dð(§üÀ;@Ø7d¿ÎÓ鿪X@
&<(zGš@­¿cØ¿ëÈÌ@ϗǿÞdÖB[3¿éó]†T(²¿éêF~OÍYUNASNone?ÝeDß$°?ʵt*‡ÙÎ?֔fà9Z?ʳD\ó¸ó?È
os÷gì?ęhMîÛ?èفz¡Ãœ?ÈHô•êà?«ËŠö=;?®Ê•%G!?ŧ5²»bA?Ãlä½MŒ?æ{­P"7L?±˜õûQ~?ÀªoÉâ8?§)M#Ɗ?ÅfÛ.%@™?¨;ðÐÙ?â¸âõ¨Õ?¹äՄ-ü?´Žäʍ×?«Ï{e‡‡½?Չ[}ß?¹ÆŒ²¶ë3FGL J1721.8-3919@uÉÑc4'¿¿øs
=³À8·5@L À:B·
èa¿þŸ>+´¹±@A
•iß@Xwœ'"¿í±6i|#¿ÒSüÖC²Ì¿áã6+h¿íbZidz¢UNASNone?¨¤/½A/?«…4i1á>?â÷«¹}Ò?ЛíQõ?ØÏ<"•\6?Ð|øÀÞ<?æ#­(ˆ=?Ö¾žÜ1?›5Ïò•Ã?°.üQ?ÒH°Àö*?ÕÎq±jS?Ç´IŒ$Ó?¬3÷œ…Æ?ÒJo–ý$?±l"r¦?àíöµÑx9?³ìµúkñY?㎸§¤(?Í*Ì?l?fZ)«?y/,ìþh?ضü´‰\?Í3???3FGL J1722.7-0415@2~µ^ñýß@1"BÇû¬´À9‡YûôÙÀ:æ+Íä$?ôëG©·ÉÛ@7´»³õ»@[ü€¿?ïûǪ+À¬¿àñ†»»¿ènÂ+øÆ¿ïÿ›ÞIàUNASNone?°üæQÕ\q?¶à²•TMó?ëÒt5àRÞ?Âғì;?°owÿ(?¸à†ÖeK$?£
X†5?´[4Q4Û½?ìg+
Wãw?À fŸRK?³A{j&V:?¸VM®Ðº?Äo¦ˆ•Ý?«ÿŽå|?ãߍ(÷H#?´þÍ¢ÌÄú?Ì%[šI"?¯~¢´å»í?'÷ñҙv?Œ0H{%F?ë!š&ŠÊ…?¹èe†§û?Á´gš'Á?·µç§q"3FGL J1723.6-3646@uîΤ¨ÁU¿Øsš×\HÀ8›EÏíé}À9¢P¢¯ÂÑ?æ%c¤·@
Áñ§w¨®@Ìh€Z?žŒä¹ÚU¿è,E·3!¿ä*ï-†P¿Û£±[¾RóUNASNone?lbPå_7?u1€	™ÚÙ?®‰w¤Ol\?¹Õ…WHÎe?íû4Õª7?ºQ²Þ3eK?µMÊàÊé?À‡'ˍ?±Îv²Fë¨?¹OvDH Ú?ë#Gp[	.?Å+éK1¿?¿üß?¤Û_°@ˆ?½ìc¯?¨#œ™<ûæ?èBâœûsZ?°'ƒeA½?Á®‹âc؅?Âa]?
?zmÔwF°d?'ÌtIoV?ë_^x|~?§ͱ†—‹3FGL J1725.0-0513@1ìh¹ý½0@0&cAøÀ9´â:¸cÀ;ÙÁfg¿ô¸Î¾¡@Û\ÁL$@%ÄÀcÝ˿ǃõ…0"¿é1̋‰`'¿àz»÷¬8¿Îxí|›UNASNone?íéb'gÓ?µh–sÆ
Ä?`R™?`Հ-,P?°5UwŸÍt?µDSžkÒ?ïzÎßû?›.ˆua?d4šoh'?i¶÷È]©?Œ?!žŸüH?™å ÕÜ?ëø	24ÒÜ?®	Ãïޏ3?˜¼=71?‰]«àæÒ0?º§.KœÝ?«ñ&Ð?ˆ?î"cY¥Fª?¢(	½#Å?£~ŽÐ?$²î9:?­Íx¦£Mò?¢%ËîR/ð3FGL J1725.7-3555c@uý—ÿCB¿ÏBwß4®]À8+Þº5"À9O·Xâ?Ýd"¼Ð@dZ­ Œ¨@Àè€1"¡¿ì·ºýþ";¿ãP¨¸V¯J¿ß‰DL`*ã¿ëw­þwâUNASNone0?šñy	ÿ)?Ÿc ý´‡Í?Ø	
+â?Ôyã{bW?ã#ê+:š?Ô-'TOJ?²ÀÃj&ì?É×#<Ã(R?»7u[Œ'?Â):Ÿ¥Q?çìa#³æR?ÎóœE´¨?¿~˜" Ðd?§'ÇúÀ?бq	?±3 lÚé–?ã·tdç¥o?³È
¸Ö?¿žLŠFw‹?Å	ј_?xbào_'?|][ÛÉS?ëÛp­ØrÁ?ł`/ÞJk3FGL J1726.6-3530c@vÑ·Xâ¿Æ'ÍúI\ÀÀ7£-0º²ïÀ9‹Àނ÷?òÄïc$½z@eÛ­m0@u¹_݋6?ìဌò/¿æÐZ\± ¿æRT­p)ø¿ê΍Ÿ:mdUNASNone$?'+ƆÁrÙ?ƒ©Tüƒô?Ѝ`LC?ÍŽ#ÍÒ?綊X´Ô?ÍM© ö ?'7"& ZD?¦pbná«?Á¦€ã1ß|?Â<²Xfºÿ?룦…O?Ä	s*Èr-?«g
',xˆ?™Þ?H0?Ñqš&\ŸÕ?µûPFß{&?åÂ®è?¶Ë½ÿµÀú?¢ˆ@|÷3?£VbЃ¹?²à#'?«pÏÛ®?ì{wˆë¸?³™Õ
|ks3FGL J1727.4+0634@=6cÇOµ@5¥yžQ?À9‰/Þê܂À;:³In?ï.ú81¤@W]"Dù@&À36c¿èEw¿çx¡È£X›¿êÝ\îSÁY¿ïùAû«UNASNone?êÅ«l?¼"…;²
?ÀHZ–íg?·©æÞy8?£Œ$¾âØì?¦£(¦4´(?ááØvZ#§?È[†u:çª?ך1sú"?Æy4œzè?²ˆv}D"?±#½TۑN?èËb7°tt?¯HÇ#8º?¿T9¤Üq?¤ªaÏtðž?ºPµ)×ò?¢¨Ö·¦_1?Ë}"︚Z?²ð
"Œ‹Ÿ?âu"&BA?¾úFfW?ʮڿ®\£?²ªãÀaY3FGL J1727.6-0654@0Á‰&"Ï@.AðÃLÀ9A 6×,¢À;>Ä`î?âÎqê iº@H³SÜK@¬M@O¦[¿âC<}‰ÃŽ¿èó|Š¿äw‹pû¯}¿ïÿ݃±Ù_UNASNone?èù]q#°b?Ǐeι? ÓSÂÔ?¡ÖZK|9?È•sœM½?Æ*ó<£Â?êl³;u?»Ú	™þ'?¸\ˆÏ&Ÿö?¬…õiQ"¯?´C9–ý´?´½@;,î1?åÀÀ
‹S#?µLïÿô3ø?¸Õ-°_OŽ?¡îÞÝÿx?̒hñ£®?³U#Ò¸,?܀Všk?´tõµC?Ä_/笁?®YǁÐmË?ÙPr	‹´?³³C_¢;3FGL J1728.0-6446@tvÌcñA À0MÛU%ÌÀ:¾[
À;¤®ç¸5?™"¤¹É"þ@YKÞzÊ!@Nº€D¿ê$­´Y¿ç8Q¥¿íÀ¢ox€¿ïýb¼¶UNASNone?ïÔ{€¾;?yÕÍb\O?cÍKjwMA?ipjÕMž"?g·4Êw?q¸#²§æ!?ía3Nàš?¸böæ_Ä?œCtœpk¸?¢æ'ž?«ËÑiÀ?²3˜ðñP
?íª6ëf‹¬?šØ'3a%µ?¢ðBw?n»Äv?£V¡5U=Ü?ÝùŸþ£E?ê&'Á'ºN?±~ÿŠú+–?³1':2¸?©‰¶ËcÙ?»2e‡ú×?¨û=pÎw»3FGL J1729.0+6049@Vr¦óõ/Â@@µ‡?úÁÓÀ:WQ§'€¡À;¢µ'ôcë¿ëMT¶T"@ÒU ˜ÑÉ@-ž_§'¿è`
rô5¿á/èSÍÜ¿ìDƒŸÝ+¿áôÉʨŸ
UNASNone?ﲄË ?‹¡ûÁ)æ?|¥¥·
°?‡,Ù<͖.?d1àéqÕU?q79ý«k?†™	?'ÉqÅ]2w?TLLddÁ?ˆ¥å2[¼?~ÚðgÕ?"
Ž6rý?íäáAolü?š.8‡P?šÕu¯
‡?ŽÂÍ7iL?¤G1"/
?'Þýقã¡?î²ÝÎéò?ÿ¯Œ"_ú?ƒ[ÝЭ!?†Š¼ío4þ?ª=Ú®åüß?›["‡t3FGL J1731.9+5428@TŒ]á\¦Ê@@"ð^¢LÇÀ9Ò®Q·'¹À;Ù
£ÇðÅ?ÜÑ-<¬·6@
_hT'I›@7#_ÖS¿çފƒu•¿ë€"È×Ë¿ëÄ@Hq-¿ïþó…?¼ÑUNASNone?îÏ#ïw>u?¤°ÊgS±-?†ñžu°?‡ªß®`­?š¢²ÖP¡—?¢b»QRb?ã¸Ø¾kâ7?ÉÝ¢TÒ%q?ÔX ψ¥Ø?Ç¥¶ÜÜD/?°Ø¶Î~Vá?¯Ò"ÀZ'?ìc­/?¤g–!>1ä?©tz…ß?"KÅ;ë?²zª0#…?žî'7*ß}?ÜL=Nû®?Ày€L挈?Ý\^êuL¥?ÁÃ-N?¹]<7?°{U…R 3FGL J1732.4-2709@v×Ûôˆ@8™aeu¦À8º­²URBÀ:Wè+Íä$¿þëÖj…Yò@"v¸@ûԀ Nj?̧¸ÃL賿ê•`;¿Ýû–EɅ<¿ç"´ìA˜bUNASNone?Ŭ³í:?Åø¶åƒ¡K?†sÙ\)xf?Œ}hæ'"?ê;ŸNRP?Æ©jª­×T?éýƒ‹*Yo?Ñ?cœ?~ëÕþ'ÒB?'C­å‰aõ?Ç"#e[°?ЮÖ5gí3?ÒE†ü¹†Õ?¶¿<¨¥–?´‡Ò¢>l? 'b˜†´•?äLB>ôÈ?¸¬zm)—%?æÛ.dƒ
u?ÄëTâ›	Ö?'°ÐƒAìf?5û:°¯?ÒF­é'Ù?Äë
:Ï%3FGL J1732.7+5914@Uøo?Rü&@@ƒô#Rë_À:úkáÐÀ<®âô?¨«CLš@)¿A@S f'?ïŽß{r‰'¿å?Ç7%tó¿ä{þi/¢
¿ÅQwnUNASNone?ïÞð@a1??wµáDŸ¬?aG⌛Ӣ?rØi›¢PR?_º$eÚá?d™èù1?ï¡vLMÏ?÷ƒdsœÜ?ucK¥g}Þ?~'ׯ´Ê«?yáŽXñš¨?‰/u ¨Ê?îßÝ¿Êh?'n J?"s˜ô-Ñ?ˆ®Í(ó$?›kSÙ§*?‡žÙ5<XÉ?îêk±	K?ŸÙ7æË»?rÑ
i`Z?{öéd'¯Œ?þZ£~–?ž	.v"3FGL J1733.5-2811@vsw[0@#lfZ§ìÀ8Ã=dRÀ:.¾ÐŠÇo¿äРÅœ´@b£S&@é¿¡Á¿ÀŠ»î‹Áó¿ëòƒ
¿åàèϦŠ³¿ã—KOx}UNASNone?ÐͲQ?¤ù]Ê]S?'ø3eÚä-? €P<Ù@?Þc˜?¯Æo½fiÍ?ãù":·Ä?ӄSÛ<E?"Ö™9º÷u?Ÿ£R<«?›?Ö¿oöö+?ÒÖ5¸²K‰?Ìt—æ#?±nÉH6»§?¼¡»Î1ì?¥ê±9Ðÿ?åN¨À"åÚ?´ñ»;¹»ö?Û\Kô†?Ç)m?š¨–?Zãôalß?Y[]›©=­?âD…S‹Œ??Ç+('µ^3FGL J1733.5-3941@uØۋ¬q
Àâ1ƒ/ÊÉÀ9&/ŒEÀ:É+üLû?ÞC+9zÜ%@­OoÔÏ%@×àŽ¾¿âr¶ì€Ø¿ê'WMKt¿Ø'å¾òTؿݨ`'CLUNASNone?äÀ¿Ã›þ?ÈU@§-b?xº8¤Zù?~-èm¤[?֝ç\?ÈU¹D,>J?æWÝݶEQ?ÏÁ¯ñ$·?=%™-)Ã? 0B›"??Ñ|që¢Ã?ÍÀ}úŒ?⚍H+'º?»¾y]á'R?®¼!ÓBÚ?U&K+ð?Öóa5@ŸJ?»:à¢øëö?ç|·n?¹gˆQ[ÍÃ?iÛ¿îUîÉ?o©gŸ¿+?Ñ«Oèwò?¹NΟ§*3FGL J1733.8-6056@t³‰ßrïÀ-‹:%•»¿À9poz^ÙÀ;'2{}NàÀX×æÜBŒ@%€˜Á­_@§©Ÿ¡—¿çN"kô¿æ-ø°R¿ì"ùTs¿¶G€‡UNASNone?ïË-ÓÓá‰?xž+6ùt[?kúãd±'m?jϝFŠ?h×HÇlôÝ?q¡#éŸy|?ïƝQ&¡?ŠÎïUÙ	?Qàϓ%‡ê?Y}PR§%é?x9#‡æe?|A´-ñf7?îVÎROƒ?"ÿi›Õ¦å?'4ïÖ擹?ƒJ"C.R@?¡x¢ïœ­ï?E÷èÌV?ïӕ˜(á?vå2…@>ã|7؟þw>ý´"÷/Þç?v+`—ÿ?°?vx¯b~3FGL J1739.9-3124c@vT&Á½¥¿Ð†êÕÌOÏÀ8\+xSδÀ9ò5ýé?õ€@tº<&@zž¬¨ë@P¿ "_ž¿Ü`7˜r¨¿åӃZho¿çd'²ÕŒ¿èߪ4ùyUNASNone<?q'•RS=ð?lZ	À¼óÁ?¼Y="¬d?¼[o³d?ìQºMªÃø?¼o¨3š]?"\MʋÂP?£ëÔ¬
©?ǎكRbh?Ã{!Ȉã®?ég0×	T?ÄÑ×TBëH?®¸n×E®'?˜pJüÍ?ɵ^n<ÆÂ?±;¢'N¼?ç§!vüsm?²×ÕÓ$íÙ?³¿–ñDZ	?°žñ®H+D?º½S•¤+¤?¯Ÿtvûš¼?ê0b¯"ïJ?¹awa¼¶3FGL J1740.8-1933@º¡<ü	Ñ@NkawêÀ9‡¸·lxÀ:ÚwNëö^¿ý133‰o@5M6¿"»@²¾_v³¿àaKw«:ß¿ç<A³¥£¿áv…¥ñ¿޽çIÙEŠUNASNone?çjaÿ ?Ç¡u²°?f[Ȅ°Ó?ej1æ_@?Ðþ"p¶`)?Æö†­×\?în}ª(v¦?°Œê`°Ï?hã	f®Ã‰?xÖM'¨ß?§‰ôÇ
©u?°}\ݪ3?æ=ùOT§?·3"§æƒ•?ª՞žÒž?œâÝ/"?ÐAò­"_?¶ê" "?î^JrÐ$P?¡Ýb(2'÷>þòOdDAÑ?¦•>jÊa?ªz‰2?¡ÜF{‹Þ=3FGL J1740.8-6755@tRg ù	lÀ2¼8…	ÀÀ:Fšï/À;»\´5ýÀy
‰ò@`›csAì@O蠒Ý¿ça¶u¿èÇÖñhãn¿á'Ú~U	¿æ)wT—©LUNASNone?ïÐ#öÖ"?›.'æuˆ?B>ÿY:»?]󻜜 ?u¦$©Ë¸‡?™Ùµ›Ìþ?ï¿LÆ$¤?¯±¿>!»?TÔ ó+¬¹?Z'zßa|?{$t½"Ã/?|±¸òªn?î·¸kF/?}+HÑ?…¨·0‰%?tz·", O?ž…¨öþõw?‹¦@]E?ï¶1ƒ¡V?zêUœ¨Ú>ù†ÛC¿?	FÉp¯ª?'gÔ<ëJ?zÝÒטŽ3FGL J1741.4+0938@@âñ©ûçm@3ãý?[_¢À9vèõø?AÀ;1ÿD]Å?íº^?rÓÿ@À9Iøœ‰@ø8`nª®¿ß؎Éöj¿ë¤g¥£	§¿èpp3 …¿ïñ'½pI¥UNASNone?êFdžÕ?¾;NøöŽJ?ºÖy\8'?µ[Voeh?²óJsi0?³çڜ/?åð}EñŽ˜?Äû!¡1@?ϝs€ó?ÁõDK"ù4?±A/Çs‰b?°†úì×V"?çX¤¥×?±·Zv­?ÁÌ:n¯Ÿ?¦L}‰÷ÔÜ?ÀÑ5*¹ô?§tÔ)X?ÒAÄ^¹(ß?´h«z¡k?ÛIw?½cûB}¡?Òu:4_¢?µ/usٜ3FGL J1742.4-7237@tgßã*À4à´Ê!!À9ùÖÌ*žÀ;¸ßR,¿ÞÞxžÕÌ@ 3&H@aÌà,¿ìé܉ûŽN¿èú¬Èº2¿â2úûM,¿å»¢ÆBUNASNone?h[=? `ÁTöJ?Z…¾›'ñî?hêëf'®?‰i¤ÒvÒJ?Ÿ¬´½ËþÖ?ï+Ù·î¥?¥ÈlËßYî?xc¡9䑜?Š£wð3I?"k÷Z‰õ?¡V¢ íõ?í¸f'Gƒ?)Æ+#?'Ï™©]5Ä?'(_÷Ûs?«Ê<ìã?—ý®aD¸n?ÍAN?š¦‹O?`Ϋ3ØG?]zK4ã_é?¥™ˆx²@×?š5ðš#3FGL J1743.9-1310@*«ø˜,²@ õµØ",À9†·5ŒÀ;
3­¬v?ñ5£Ãi Ö@ó»Æû}@ærÀ'Ö¿çpïñü¿¬ÍÆU;%¿äv–9½»ã¿í¬ŸâKgUNASNone?²1¶Û^!?±é/à-?렌+×(?»D˜ìʟ¶?°ÉèkÈ¡?²Ÿ¼…chÄ?ÞS¿Ë猌?ËkúÞ@^?Ñqðﯭ?Äc­TNYµ?Ð:P (ÃÇ?Ɩ¯KèI°?ÖêÂTÚb?¶æ;o;¦?ÝuÄã¦#Ó?¸
lãÀJ?Ç>ñŽÿ'–?ªê)›öxÚ?Ö\å÷`i?¸µp°ßD"?݆¸ûÈIV?ºÀÒçÉ.?È8Â^¬ƒ?²¹N@J>?3FGL J1744.5-2506@	0"¿íÁ9@¤±«VçÀ8&ÆÌ˲À:)}uv¤¢?Údúr™Çß@
Ó:ÉT;@‡À(N©¿æšø2šö«¿êñísˆ¿ã÷[ Üü<¿îart`UNASNone?À"Ÿæàa?Â1ÛO–¦3?Å»ìò7:ƒ?Ç»J5…Ȇ?ækÜɺ?Ï5ïÕ{?Љò~ñ?Ëð5ÚÆ|?ËF«Ÿù°?ÄޕfP¦?á Z>Â?Î! ]R'i?Äúzí5?¬kþK;À?ËƦèao—?°:iš-1?ãÏÕç@(Í?µºYŒíÇå?·Q±G\ŒV?²kAAò»œ?³Rp;Åí]?¨¡•JB†?ê«{ϛ°Ê?ºÈúbOÊ3FGL J1744.7-3043@vfÃóà7¿ès ôlNÀ7þ+i:V=À9Æú¤vln?î&U)s@F¬RÐÝ@æ›_Â]]¿Þúê—c	¿éðŠtÁ%­¿äÞ—fñ¿èÕ¨5
EKUNASNone?‹‹$Ÿ}¼?Œ<ë|feš?³Ç	¶ø1?»1·VˆÏ¿?íòxŽ~£?¼ÿ©	ï¿?°¥2ý/OZ?¹Ô£¬³M?Á'ös'n˜?Ã!<wó'F?é¡\yzo?Ça6à{Þ?¸ÔÖ_¿\L?¢åzd[±³?ˏ/f`'e?µ[ûŠùŽ?æ™ZoïÝ?¶øÐ|YPß?½|ݗTÒq?¸æ­ZÓ&U?–ZMÌusH?â:ôa
R?띑ޱº?º—ì³ÊÙ3FGL J1744.8-1557@&™»'ˆÛ@€ô"'òÜÀ9Rìzçý«À:î__áçç?å+Y Çd@ö–²‰›@z‡`%¿©ê7'õƒ¿äõþš'Ö<¿åjc㡜ë¿î–"	u°ÂUNASNone?¿¸¦¥Wäo?¹3­¯‡Ý?ß¼¼q¦_??ÏHcŠ°Ý|?ØU姥?ÍçUÊ"õ?Ê:5ª»?ÄnáVJ"?×ìF:5^d?NJˆå§T?Úö«¸/Ì=?Ê0œ¾¨+?ÚT³ŠQhÇ?³¯B¾Ö:6?ÐÚ°4ÿ'?±܆n^?ÔМby˜?´…'2D¦?ÃðÀèó?¨™JFZV?Øïǐïîx?¹óä§z¾ß?ÝN·ö¯?¹‡"6¶*S3FGL J1745.4+4721@R'±F^‰"@>n9`sÞÀ:'ó²ê£À;Í
ÌÜ­À÷l–\ò@ªõ «†¬@wàyQû¿å`üŒ&¿éª¾UÌÌ]¿èHˆ&w'¿¨'‹‹ïøUNASNone?ïú¢6Ûç?K‹slq/í?"Q8ùXPè?#`çÐWÿ´?C(æ:P?IÿµPi}?ïËB†¸æ?‰ÈÃòñæ?_wUç MV?f
Ü`ñʍ?r»y:?ˆÙÍß«Y?$ò¦Œ?yèæJŒ ?r¾JŒþ?iaši9©;?…ŽžI–}?tçת+ßj?ïüIì!q?Dº''ŒC>y[ˆ{˜o>ŸÃáæ"Ô?=¯	;ï]î?D¹ºÙE?3FGL J1746.6+0433@="¿¤Æ†@0}­ÙÂ~•À9œ-~¾LÀ;*þ±KÀúð¦ñ›ä@
{«lù¨@Ys_ÉZ¿åÇ\R׿ê¨Üäá°M¿ÚÖ\j[Šã¿é–è4l×UNASNone?ì€4Œë6?¾¯ü\ÑÃ?v^ï'ÄV?wÖÂ
+ߓ?º˜zp/Š
?¾9Ñ&Ž¯?ïZ»ûü×?¥¡ßÿ?gõñ©ßHL?qíìÀNY?'©ÂK)4ž?¤hþd<?ëI̐Óî‡?ª:$öJ|Ý?¡´CÀ,Ë?sg`¾&?¼×y™JKÝ?¦Ü.t€A?íÞ°.ÙvÁ?¨•mlùš
? îw.ÈÓE?0'jyß?±Mœå–?¨©'`bz3FGL J1747.0-3506@v.cÇOµÀ§|{{¡aÀ8MRÓâjÄÀ:²	Bžá?ãšÛ—&3@ª½ÐZ¡@UÝw"q¿æ}"®î¿éÀ¬cÜÚr¿æa¶DU¿êaé©sΦUNASNone?í­ålÜ\?±Il뀃? (ýº &?¢ÄÍÕ¸úb?¥€A¸?©Ä?×´î…‹Ø?ÐÖ"àC"?ÂþÂpM‡?½5Æ â?ÞË°¬rÍe?ÍÅgØc«Í?áD´c&G?¹Òós+Ÿi?ÆU¨Ã ƒ?®Â?(Ç?ÒnìeQ¡?´kB'zŸ#?Ú(Æîke?·Uõž9C1?²
fò§? ¼\0tÇF?à¨zç= ù?¸?ëªL¤3FGL J1747.3+0324@<›0aǛ5@/—Õ#³coÀ9iRÍ,nÀ;âµl]÷?¿€3¨4MK@
ã¤)Àn@Õ€ÙY¿æj2X¿âZÍÖâû¿áb¾Mz~™¿îWÂ?'K©UNASNone?Õµd%H2?LJ=DÞ9Ç?Þ³õpÒ#ã?È´ÃCî˜?ÈpªV'Õ?ÄbOÃb1?ëj —ò©R?ºÆr)vñÖ?´¤,;ë‰?°ÊXõ?°Ï•á?±dÄp,™?ä'Sg«?´'WZkĹ?Éܹ´g'Õ?°P²A4JÁ?Ņø¬ìi)?«C˜škû-?ᑟcÌÁ(?º¤ú´ã@Y?¹i x°?«>SŸ‡f?֕&ðHz?ºy¿±:¯3FGL J1747.7-2904?À&'j(¿ÞZº LѕÀ72_½‹çÀ8í¸_~?ò«Ð}ÜO@·ýÊñ€`@ ?Ðû[¿â'†Là®V¿åÐ܎¶¼•¿æƒú¢Ý÷¿ê¬;ۀøAUNASNoneP?Šò´™Ýu=?Þ¡]ÚET?Ö*o@~½?Ò@€Y?ä~ýQÊÌ?ÒWå—fNƒ?¶m)"X2ã?À›3y$щ?Å{šów…Ç?ÇU$†²?çÓt·2?Ì¿±¶£?»vD5(Ñ?¥x+²áÃ?Ó}$Œ
.Ê?µòìep‡?âÒ¥7ôC?·JsC]¿?¢oëNËc?®¡éT"Œm?''GøkM?'[Më-Öô?îS^Á‡¶Ï?²O¶èì3FGL J1748.0+2701@IêÊÿm3	@9\gßã*À:H—hfñ§À;ˀ
|ZÄ¿ô=$*ך@
֛	Ü!Ô@8Š`¿Z¿åùzíSwn¿àC8P Îº¿é¹">o¿Á¾ºì¶³AUNASNone?ï~‰©z_?"ðMÜ}?"$zy€i?jÄ<Å?xrƒ¸Aý¤?ƒä˜ó*êÆ?ïÇļB?ºF8ÜÜñ?eGUŸK†"?kŠb:!Î?qy÷"¸öP?xU€?$9ñ?î6
ÙÕ?—·³—*?˜ÎœpD<ò?ŽëÔsŽ]$? 7àÕàD7?ß4ù"?ïĨL,
/?v*÷Α±û?!r"hꦸ?0"Q۝?} HÖ²$?vš·y3FGL J1748.5-3912@u÷ù=ÙcÀAhr° ÅÀ8סÙÙû‰À:ø
ºÓ¦?ðofÈ61@œ4¡rV	@mŸ€8t'¿évq¡Wþð¿Ñèß	Ü5¿ç­o÷¿ì¨Ð%Ǻ¿UNASNone?«ÿàK?k€?«ÝÉ"='?ë˜NÁŒÚ?ÀÿT‡ú*Œ?µ=ŸSãl?ºº'÷bTC?À¯b¼P1Ó?À«ˆË?ØUØR°<C?Ĥñ4¨Œ…?ßRvO'ªÕ?Å£›Ãf(?Ñ1cù)v÷?µb`OVÁ§?Ú÷SÃ4f?·rÔ§¾½?Ó×HòT¢?¸¬Þ¬õ­?Òy'GCp¢?±»OB㓶?ÜMÞHr'?º¡D¨æë$?Ñ9wÚtÌ?´ˆÄ½˜ú3FGL J1749.7-0305@6ú¾Yl'à@(o:¼"peÀ9,AˆaÀ; ¡`7x?Æëñ•®þ[@ß9Xç!ã@fÀ_ñ¿ë Þ®ÁÊ¿Õ@ÆÚ'w¿ç‡½;èÁþ¿íË !³ƒûUNASNone?Ð¥^;Ïì?ÇU³•"e?åÃz¥¨Ù?ÉVˆ³lÄ;?µdk>‡yƒ?µò.3QN?èx¾DÍf?ÆHj$Ä7?½åÒþÙ\?¸iwÝ|«?Àë3‡€@¼?À#·]´š?ÞÍÁã³¥?µ©Ýp<=€?ѪªŽ‹>Ã?²ao·Þg¨?Ï{_"1?³êÛm_I?à4JN*û?¹Z˜º.{?Ê)#êˉÄ?º'.$Å?҂ÙnDD!?¶éR=ò3FGL J1750.9-2220@ö>¶5@ðï ´«nÀ9³Ët9À:oóþj¿ýQÃI@eÌ@AþíÜ<@¤hŸÑ—¿æ6ÈG'¿íáÇï~Ž·¿¯¼ äôXN¿åO¥&À‰UNASNone?҄€WÐZ?а-Âc¢*?jßäÛj?tьMb m?æ¢àÈ3¶$?ÐÈB؅V?Ù·¥ùäî?×ã@tǍ?'o‹#m¯¤?¤$1Qxg?␰ª` ?טjÄø"?×£¨¡Ýl?¹ EñÃÆ?¶:¸\­Ói?¢áéÄCž?áfÔíVÜ?¹Õþ$Ê,?êpÈ`0 o?Á5¿ŸP¥>ô£i0^d?ž›†N×	?Æ<9fd4Ä?Á5z!v3FGL J1754.0-3321@vQú¬Ùè>À'å=ÌÀ8çj"ò¬À:·D[y£Z?ò¹ÊE
@­\7äH@K?ëÓM¿Ëý4±ëþt¿êGVù'¿àÜÔ2Wý(¿ìý‹UNASNone?؀ÛÕ©2P?É&-÷Pú?¾pÏ,R0ô?¾(ZIÏ
ž?ßâð_BAt?̅tåK#S?ÔmŸŸß—¶?Ð:?ft–]?Á¼}ü-qa?¹Øˆ^ëvÅ?áZ±×Í?ͼ3¨Þ³?ÖåÃIÊ"?·¹:ðc>?ΪUL?æú?±ßà'<Ë8?ÙÅê?¸Ÿc­ò?ÛbäzÅò?¹S
à¸Ä´?²N™ ^|J?¥Ý½<Û?à+{i¶Í~?¸õÒ×&®33FGL J1757.8-3126@vsC•Àv€®ç	À8ÞæïÁõÀ:¢MùÇ?ïÝæ"bè@
6ÐfŠM¡@[,å¾`?ýGªí¶ž¿é^¡i5Š¿ã¹ÛGR¿¿ìÔ°Å@w¦UNASNone?˜E
^?\?š
9*ÔW?Ò3æ^ExÝ?Î"O–Vy?æ#ãðŠQ—?κéÉMR^?²Ç
µù?º<£¢4yï?Øjâýb?Ŭ®ä¼£?árøWÂ+?Ǫañ1ì?ÂÄ~ËËð?ªfµP²Ù_?ÒàVT¤V?¶xù€hº?áÞµ"ºØ°?¹™©J¥;–?À9SFœ4a?ª
W*•B›?Ê-Â7"?±¿éþšåÖ?åqŸìèe?·¡§#˜æ'3FGL J1758.8-2402@á•a%´Å¿¦7½D†À8c˜¢ù"¬À9æ×5??ðíäI–!@Yi}È?ÿæÀ'¢Ü?辶ÈèLì¿ç&k
·p¿ÑgîõX8¿æžºM8UNASNone?–¦'Ì9•å?ž"Qø…š?\Í
*L†?Š¸ ЇÅ?ïOƒÞ·?£š«J»?š%û"+®?«N_H²Ž
?¢­V+všÜ?¤²9ò9ê?îíkôö?³YžNü±?ÂОå"gZ?°GÉ&W7?± ªòA?ž_•¥J7?éÃœž?²òªYDæ?Ã=ˆOÈü¾?¾Fö"·åU?Š¾~øÈâî?¿9†W§?êÅ£ð*E?¿ŠoãaÄË3FGL J1758.8-2346@ÈëÌlU?´Ê¿_»ýÀ8^@'7|À9Ǩ§b°?ó›÷Aë]@
Üçl`Px@£¬ "Úƿ©ço?ï•ç·B¿äï]+»Uè¿ä&VÅ£RUNASNone?''l"	:Ô?—‹q"µ?ÆÆ(±;';?Æ:ü/=·n?éºboìZ?ÇVtMéÏ?Á,5îçýé?̧ىÆ×4?߈L£Çl-?Ò<b0tù?×á˜dĔÞ?Òí/Ô0ˆ?µ'IvÍ?¡®èÕõÓ?Òó˜±%u?¹ –§•¯†?ä@Cªx«?ºi"'Ú?¯yJ¤pQ²?°bÕÿÃ4Q?ã¤&9cP?ËZx0W?ÔȊ9E/(?Ëïà—6÷3FGL J1758.8-4108@uì²êòÀ ÷W÷7ÚbÀ9Ÿ"!°SðÀ;OrSÍÝ?ð9ýŒÞ[@¨¢?¢§@ÓÙ m2Þ¿ÝÔR}%o¦¿›÷Dg"¿å÷
€û¿åm|^ªöUNASNone?êˆDkÐL?»lÄÜ2k¯?±ÎTý?®ÂùfóÆ©?º·'L€?´£hy½VÁ?äÑ7ëàãç?βšw Ÿ?´ÈžE\lE?´a_¦Á·Ê?Ñ+h–ç ?ÈÄ÷E³&?꾉/'?ª}]D†D?´"œ˜]9?Ÿìúµ~!?µŠºãYr3? ‹Ø&ȱ?ær"^–%?²ùy¥•Ù?Å3x*òª?±€/ÖJê¤?Áþ]…´Á?¨ÿ¡éùËv3FGL J1759.2-3848@v0@9«óÀ´ãy·|À9qiiP%²À;ö¬š'^?ôÑïK|Ö@×ëϜ`@ãéÿ"S?êužåÞÁ—¿ÞWí',Q†¿àRcz¬L,¿ïÿû)pU—UNASNone?±ÖMˆé?¸èØDø…?ç,kˆçÁB?ÐYöŸÐ?Êc	µœø‰?̪õåaÓ*?‹Àx(É"?¥Þl¿_Š?è'])©'?Ç°zKR-?ͲOQ×/?Æ.È,Ë?Äz®d¯?ªµ6NC4?䲟/àҚ?´oIKÔ̏?È»'gPé?¯§Ô.÷La?¯ØW7ŋ? "·
E'?æ‹_3½~
?Áî=ÅX?΍<v?½U´¡"˜3FGL J1759.6-2141@dÁr%·?î¾UíQÀ8ªO¨´¿À:0``'çÏ?î4)¼«±8@ò҈"£Ä@Ks«¿ìMÃñö—¿â¦â+]¿â¬Ö²°¿èö® þìôUNASNone?"l1yZõ?‹a@›þ"÷?À€sªþM?ÃO-Ö	r<?ë«o/Ø!?Ãù.ùœÞ?±Q{±Õš?¾–ÿTtýï?˹wŽÐà?ÀtÔQ[¼¨?èòâ+ᘇ?ÆÊÃ¥ô>§?Æ÷ îÅ
?ª¼Õ
ìb©?ɊŒ"~H?°ƒâÓöp?ä^4»¯+?´
—aý{í?¿Ø™šƒ¸?¸þsµýl'?¶Uj‡6›ò?ªfÿ¥ÿ?é:?{Èʊ?ÀbNe#3FGL J1800.0-2955?çò–öQ*•À	¼©ïR2ÓÀ8®ñ7æ [À:k¹8›R?ò¦©½S2,@Å2™Û2ì@N5gÙÙ¿Ô­æ¡Îá¿ê²ÞŽ~ˆ¿ë'ÏÐã1é¿ãʎÎ([XUNASNone?ÈÛª¨àá?ƊzÂR\?ÃzB…8Ê?Â÷¤|è6?äê"ÏW9–?̔ð jà?Ôéìzêû?Ò;ø*n?ÁhÝ®é˜?À!i™d ?á0ÒVÐq?ГCƍ?ljþ«ûB?²n€ðŸßŸ?Ç}vtOí?¯"AƒÉö?ä>"¸'Ì?¹0>F	?ίiþV>ô?»Ðû*».?º·,Æb?µ.ß×î<?äýC¾d×w?¿=IgF¿3FGL J1801.5-7825@sµ4'¾‹ÁÀ8b{öÀ9t¢ŸÒ™À;?Mó¨Ú¿ë)Ԓhø½@ó*ÁŸ@	òŸÅ,Å¿ê[i1¿7/¿ç@.·V §¿æ
Ðl-j¿ãOïáêtUNASNone?ïý1½° ?4†,SÀœ¤?""Հ6Á?Êò'?0Q	ÊrõŠ?1µ¨\@é ?ïÀ÷€2‹ú?|Ãÿ¼¬Î€?S)2\Ÿ<?Xã‡DÍ?zÁ5š"ۖ?yò©ÓCz«?ïBŒFzé?'QM07Û?z‡ü^ˤj?pBÃ4~W?'O_}¹Ð?}áÅHžs?易Üóۉ?{—ñ¢Ùî?^ƒäâ?!'Ÿjý&v?…á»Aá?{}óqIàº3FGL J1801.6-2213@uw¾}~±?Ó|½U`"¥À8ÔQ ˆ6À:1sˆÙ?ㄾ2Ö"@
†ÆÎ[S?ÿ{vÁ'}?ïò"c"'¿Õ89Wd•×¿é'L"5à¿ÃÀdÿðUNASNone?ŠiëÕ`?'Ôò¿!à?­26̼?´I{t>˜?íĎï3Dé?¶k¥/ý?¨êS›Í'c?¸¼_ƒã@? Pæ;hBC?¦Õ†…$?ílLbŒ£¶?¼éã8½t9?ÈÞÚ¥-E?­<59I¢ï?¿gA¹óV?¦Ëð™èYÞ?åØn}pP?²²×óB£?Óz[!þҏ?Ä3gÅÄ?¡ÄMù×?¦K?1‹P?å2V*!›?IJL¢²G3FGL J1802.4-3043?Óqº™MÀ7%_5½À9?»vc3¬À:ÞùN59?èÒD–ï@
}XsI@â°À|²X¿éþ*7Œa¿à"…‹ð¿Ñ2©gR»¿çy‡‹ÉDUNASNone?ç9užê?ǘh¿4£ˆ?¢Ò§tF
1?¤&ÿ×:­?ÎeªrÕO?Ʋ!ÍQ?ÕD6ë,ä?Ït|keÚ?ÁkJ_"yý?ºlƒµ{F?áò—‹?Ì«Ú¸¿à?äŸ`¡d°?· Ö²Ôe?´
ÆiT'? ½®ò﨑?Ѿ;Kœ«—?µ/o¶	-?à–"RÆC?Â%\Ê>÷?¥X‰+ԇ?¢Xþ±'?Ü1NIN~ê?Â65ßO;š3FGL J1803.1-2728@	ÄÙÆ°SÀ³#»ÆëÀ8õ	¾ºÀ:ŸŠÙv0?æàK£R¼!@0î™Ñ!ñ@°yݽ¿èBšëdx·¿ãðd@"»V¿ç
zÎ
¦¿äâlÊ갟UNASNone?âþ '"""?ÊXº–GÞ?ÇÿÂ®[?Ë}(¼P?Ìí,*ÿS?ÅDü(÷>?àöåÈY?Ó3"hɝr?µhˆ3å«?·Öˆ}‰?ڟð5uã?ÑBÀ€s‹1?ݹôZ;÷
?¹ô¦œ%ý"?Çh,«÷3Ó?°Wó?֑õOÈo?µ UJ2ü?ßý[Ĝñ?ÀɨÔ|(š?¢׿åþ}?™Ö#+½?ÝÁ‰CfO?ÀAsÙK~3FGL J1803.3-6706@tmã}é9ëÀ4^,ýxÀ9†‡OêùÞÀ;§âïÙ?âÀƒ!w@ΰýŽa@»_ÛÝ·¿ãâ݉¢D}¿á-0K'Ï¿ã®1]›¿éí.ÔßôUNASNone?ä£ü¬?Ç) ÏŽ"ê?łØ0ƒ"?šO×8¸?Ê!³õ?‰½?Áf?bð¿Œ?è|BV°…?Ãy´¿Qa?½s;@¿Vç?·²ŽUBw¯?¾ª²k$î?¸ÇZ=%å?ê)R-¦ðz?­Œú0æaâ?µ¯ù¹
?£Xdg+M?¹tÙ¶o+?¡¨¡Š–Ʀ?ç‰W¯¼Vj?±n—°z­[?»hG|0Éî?¥˜béx9?Ä&}'öA`?¬çMßsoé3FGL J1804.1+2532@IÕcíb@5*ò¥¤i×À9Ä*lEÀ;˜€LÁy²?ï¼ú@ÝÂ2…@µŸe`'¿äë]ÃÌëM¿î›"rëÚÚ¿Â5¤"ÿY¿ïÿÓÉ&‹@UNASNone?îÏ ©«Y°?ªoÇlxCè?ˆ3Ð[ç?"ï&Ž¦·?™ò[âfÖ}?£Ço'ý‰R?êó"ÙØî¼?ÃK_X¢i ?½¢'B‰Ä[?Àa¬U^™"?¥'Ý]‹}?©¥
	´Ô?달d±ä?§­wý4˜¤?²šAtŸá?ŸkÐ?HçÀ?±"˜ü?*?÷¨Çbs?éÁñ""ˆ?»2·§ ¸û?¯¼<µä'?²vˆhi,?Á	,sÁü¿?´1Ò‡3FGL J1804.5-0850@3¦Rz WŽ@ôº"»äGÀ8¤3¢Ä»†À:¿b֎í?ÛÆ:{?Ö@§!lŒE@þÏ@šyé¿ìâAa&ê¿âÅÝCVZÄ¿á"
ëiß±¿èÍ/UNASNone?ë@
"SÒ?¾ÓdÇÙù?™Hßù·?™TÀìEÃ?¿­Šµc,?½Ù1Rš®ü?érÈÂ@Ë?Äo|Kz˜?˜ßR|^?™q©¤ø¤?Çòµ{d?Ã.sÅ`??äðx"ˆT?¶±d}rA?µ,½dª®?¡5Ÿ¨Ìš?ÐÔqÄ®?³bh±T•?ä!XL¶.?¹&´Õƒ? "‰±õ©?'¢¸2ýQ?Õª¾0U-?¹%¢Ç_]3FGL J1805.9+3407@NGæÿ}ú@7¦êÙ'N#À:µ7"Ñ‹À;£Ò$ûb?ҜkÒGFL@3úkU9@Êî «†¿ãå~'*ð¿á©›yÙ¿ë‹<7yúÿ¿ïüO¹ÑlUNASNone?în®€N?­sûÍCDG?¥£ßà 4Z?©šÁ›¡i?{Þ©º×MÏ?›wXâO{µ?î8t"q¤š?¥(§"ZIÉ?¡ªYNs§¿?›iöˆ'šá?•œ¼Ôä:?™B×áwJ?íKþ«@?Ÿù÷eÎ#I?«šZçE?™Ið{ÈLw?ŸKtÉuž
?‹QÂNëDŠ?éA²1Šªv?´N?ˆ"%¦?Á'v{ö]"?³ޕÒ\?³£{½ñP?¡¾h\Z3FGL J1806.2+2744@K"BJ'k@5ƒ
®>lÀ:w`‰­"À;¢bAQ?ìßôi@X@!eIZçØ@ÆlZ(@?ÀkQF;¿í@Y?¿Õ¿†nª¾Á¿íÞES­b`UNASNone?ìPžÿE.?¼*ôu³~?´çlçz?¶,๯ò	?¡'×.ª+?§s2~‹"Û?êDFh'Á?ÁWÖ1M³™?Àîœ"ä?¼Îæ…W_?¨'0^´?©VÒ«Š/?èh$õW¼?²"dö§g?Áo.õÇ?ªz-D
"?¹àÖ4é֏?¥­ÀîóM?åÌï'N?¼)²¼R‡7?¿ò9Zé ?¶àKnÊ`?ÈÓ'ÉS3?´ÝçédS3FGL J1806.7-2451@"K3ÚùÀî['ÍÍÀ9;ofÀ(zÀ:ywÞ]îÉ?èÞÎÆ2e@
×Tª1@«å÷1¿é–´~¿áP²êšàc¿ìÖ;Ÿpý¿¼ß¢-«¤UNASNone?ÑY´ÁÙ?ɖZ=–Ö/?Ñ|Õ‹õ?Éùs)nQh?Ýe¿H˜?Еi\eà`?ÖÈ_Øm?Ó=Ý%ãb7?´ä['€…Ä?¼ÃˆZ'þ?áÿE£ë'?ҜÀåÎK?Ö
áM'??´>§´×Ô%?Ì;²+µš?²ÄÚ~8?ÛÊ×íô?µD;x†|,?áëGYÞOy?É ã.!¹?˜lXžœâo?¤±Bph½9?Ú¢«ÂY'é?ÈÊÊX*%3FGL J1806.8+5346@Ty
®>lL@;ÿ:Þ"_¦À:#éõÒ"À;ÛzMÝÙÀˆ6Pôå@Ô(ú@@… =w°¿å«lˆûwì¿çÛ×ϊAb¿êy£¢†þ? îÒº…IUNASNone?ïü¹3ªÓ?<°;–¿l+?'m¦#Ü£?.¾·ÇlbL?,ÿ®·ïœ?3JÚJ7ð?ïа"U7ô??F3­M?`Œ¡#??eÈ¥kI?nÂÚ©¯éÃ?{¼=b"oT?ï‡'H²ñà?{Ñüûy
‹?uúÀ\oùË?rK°3¦éb?ƒ8Í¥‹?s$}§d7?ïø~«É¢?R18ÀÃRy>¸yìáê]>ҟ™g‹r?Mùã[?R0
÷9Í]3FGL J1808.4-3519@vM—á2µ_ÀsV?§µ¼À9¤qJÅöðÀ;8ñ±ˆ¤?ñ/áo@
È-â¼MN@xÀ`'̤¿äñ-Çl¿á"ðŠ—=¿åp-ÇZêT¿ïýÁÜPDÞUNASNone?»[Á0sTç?·¥þ5(a0?âú¯ýoš?Ì´L¤~?Ó3¯¹ï'?ÉÕdó&e"?IKìÇøn?£t0¦á,?åύ¬'aÏ?Æk€ÎúÒ?Ó\Oè¼Ü?Å¡XÊRuK?ÚtCÒº{?µßh‡ҏ?×ô†¬
t?µ«Ü鶨h?Ë.kpÕ?¬cKMªþQ?µ¶¦ vn?¢ib2d?åÏ]ª—·?»ô?ÍçƒIeí?¶uŸ:=õ3FGL J1808.4-3703@v52€ñ,(À `€ù£wÀ9ݛڼy˜À;^G;'ô;?òÁ1c$g"@Õ'X3¼@‡¿¶cÕ¿ÖáY«[Ò¨¿Ü× ÕË¿çKbã鸰¿ïÿmäñUNASNone?¸8±zfÇ?¶µL?åK¿?å¯
`p/?Í´À¤Ü"ä?Í'qñ'ã?ÉÛGæab–?©µûìH?²]ª'?är"ÊC?ÆÈ0ŠÈw?Óø#¬yéã?Ŷ/!0x?Ï·97Ó¥N?²¾ó<¾¹ç?à`ü)1*L?¸Š¶™­¹-?ÎÄÖ#g±ƒ?µf/Y?¿Ø4+G?ªj'ïþ?槿›s4o?º·×
¬?Åt熤"?±Iޜ«<o3FGL J1809.0+3517@NýéÀ"š_@7aæÿ}úÀ:&Nw\WðÀ;¬GðY™Ï?±|a9L@
ƐÃ/@‡þ¡e–¿ä2‡»åc¿éÊ'•_!¿ÝÑnµÈ×Ó¿à¥R­29UNASNone?ïJ¡%²/?§tìýÒo?RÞgÎtp6?*©ºVGÂ?•}ôÌÒÕÁ?¤cüau±í?ïƒD*/Z|?'z‡RØD³?|\TµÇ`?"LJÑ17?ËEšT?‡Š¤ËéH?î3T7ÌO?–Ø'Ϧ!à?Œ+Ïd4Ýò?zË2OT?¥Åãv‡?"†
o¸5ø?î/Lsò†?™‡P°B‡Ö?q!•pC9?qÏ{.ˆU?ªçú¿Ï>?˜¦½b³žP3FGL J1809.2-2725@S*I¥ÓÀ	í9SÞ¤À9X*ˆiÆmÀ:Ññd[Ê+?ìJõA` @þ~^@x›_lw"?ïÿW'rúb¿ì>Úcì¿֡Nõ¿ç[k•>.ÿUNASNone?Øñc""o?͹éjÎl?´áj'Vƒ?ºŸÉE?àë!kx?ÐZˉ?Ô"݃oæö?Ð軿sÙÜ?ÅS%ê¨f°?ÁªõÁ~'³?à™ÇÝòÙ?ÎÓu܋üï?ߑø⑚ª?·¢=àÎ3?¾láåvG0?ª…¸:Â?ØÒΤӉ?¸^óÐÏ.ß?ÐãУ6u?»ÎàB¦-?²­·Ûθ?®èd ¨¾˜?å˜`²êï?ÀuþKã3FGL J1809.2-2016c@$]7qÁ
¿Óï]ŸˆÀ8)SÂóáÀ9¬†2´ˆ2?à¬Dh@
í÷ßõôc@›&@©¿ãVA`{‹¿éÞ)å¿æ"=Y|Èþ¿æÜuþ†GUNASNone(?SP7{u¼}?XœqXÍ?–/xЄw?¥Ëq£†B†?ïDÜ#KÀþ?¦+"fMÅ?ªތè'?µïRN¿#?¹á‰W,Í?¼ÿÇAÊì?ë#ìKÞ5?ÄP…±?¶^ýFŒj?¡M^ß?şº=¡?±ÃÌ{*?çÌ1Ñ®	
?³ÅÙ&o?³Þ¤@ž?·[¹×uŽ4?ª"­E?‰8i(Ââ=?íÄÄI‡?¹?ëØß3FGL J1810.7+5335@Tq´ör2@;h}ˆÁÛÀ:|¶ýW¯À;ÞH'¶þ.?í&/Úc8_@
Ç«äÊÅa?ü{óI"¿ïþ§UCÿ3?ïôù&Ёì¿ÊÖøwG¿âOEèÂv³UNASNone?ïâs™?p`xFµço?cÀI§?g\DP…7?S˜¢L™Ë(?\kqÎ?íf;&%`?³UjƒÀg´?­ÃLý;?°X²?—²|¡bÞ?š¬S	
ŒR?î,VVÄK?œ¥×6	‹?š^3˜CÄö?cì¢? €ÓØÛ?"ñ—萡?ìc—DW|.?³ÚäÅFÎÊ?¸°Ø=Â+¶?²ÕB‹°~b?É¶~Ëh?"à$÷ˆw3FGL J1810.8-2412@¦ÚhµÌÀ2J…_OòÀ8Œ°±
S¦À:,ñ.?õƒ-œpc•@'¡ùxƒ@—1@"ÅŸ?ïþßF]C¿èÏÊ÷›¾ž¿çHìÏ¿é/ّ×-yUNASNone?µÌîÅ)Ԙ?µRnÚÎ?Óĵš ?ÍË\'Ž†?ãÅÿÌÖx]?Ï0dJQö?ΨhU°?Ïø5…ŸÔ?Å8vi–Ð?Âá^´]"Û?ã+8aßÄà?ϧ}ÒYo?À,I¼Íº?¨¢1g  ?˖+gÄû$?±nU	{F§?åb¶ÛR"?´¾:E»Åå?¿œ
¦R?²ù±šälJ?½Lú®¢(	?³wþ†œ?èbß	–ð¾?»¨‰äFÂ3FGL J1813.6-6845@tY+jçÕgÀ5ؖÝ&·$À:0ÅJ!ŒÀ;¸¨Uôÿ?ë@…ñh"ñ@…ÖVÍÂ@9þgú?º'¡0Dt¿ãn¤ç?ó¿íDTd ¿ßHQŸÒ:UNASNone?ícp\ EÓ?´üÊðPBã?®¿ÖòV3¸?±öN¹Z}?–F—JÞ?žÌêÏïÿ ?îgŦÝ?°•QÏUìÕ?ŽðÐÃLA·?šDÍút¶?¡Çqa[Ï?¨Pk-Œž?ëƒPdãô?¥þ²"Ù?±MaÒ¢
ý?žßë'ˆà?°žƒª6Õd?™}4ÓÿÈ?é®îÑý?·~¸ð?µg¸ú6‰?³22Öj¼?½ Ð}aÿH?°£:Ýß3FGL J1813.6+2820@K¡rGE8ï@4,ÙÆ°SÀ:0"t¼jÀ;¯M†›¿¬vä"`@
EiÁƒ@§†€b;	¿äj4Z`ÚÇ¿è=&ÃpX¿Ù± ˆ¿ã%ü¬,'UNASNone?ïbã
äOÍ?šµ@Ã1û(?HÔß
]ÒÏ?IÒÝ~?'Ü÷«¸?š["‰O?ï€Ìéý'£?ß•œƒY?y§À‰¯?yuí$ֈ‹?ƒBñ ZÉÌ?‰`Ç^…?î©â¨6?¹¸_.?†ÊCÈöï.?vS³"³Ÿg?Ÿ^‰áa¦?‹u"'JôQ?îMWÅî?"Ì4Ð뀲?hÃÝðY?gq0~	Î?©£Œ¤®C?"6Œ§±Ä3FGL J1814.0-1757c@)ƒÅ›€#§¿Æþ§°³'À80RÆvÀ9ŸY—K
À?íð}ø9žC@NÎLBy@s&@©?ïþ€ªú¿ã+…Æ9F¿â—y';|-¿íb=/òr4UNASNone ?z¿`†:}´?}Ìõæñ?Ì	îåÒy ?Éý	‰.Ö]?èÈ…~ìž?ÊIw°Œ?—§r­ÿ?¦øýuö?À¨µ-'?Àdjæ@<{?ëQ?×O\?Âɲ"aF?²füi§›6? w7›/À?Óçt¹'Ÿ`?±èø¿sJz?ã¿f¼é?²¾Ÿ:öèr?¨sR‡E¼?«íŽÿ̹&?®è²Y&!?©òrM.Õ?쏍¥E)²?¶í¬¿v·^3FGL J1814.1-1734c@*5¤i×4/¿˜¡©¢?hÀ79™J¿@óÀ9tõɯâ?î:ÕG*ó@*bÐYÊ!@_R`u
Ä¿äüoÞùäͿ菪î^J—¿éÔnÆ $¿éK;eé#UNASNone`?~z֏á{?€Ðq^‡?øižßÙ?Ç?JQ ÆN?êÿ\8x…?Ǎ
M¼c?'ž‰©šš?¡8:5´&?Àï}°Â{?Àݲné	?ë70O­Â?Âr°F-v?¶:XÑqË?¢Y¬ô)tø?ÑöÓé§?¶Ê-±†ø?ä=Jðþ??· ˆãr?¤ï 2Üoá?¦å0 °Ä?¦ÍFotÐ
?ž¼‡ÿçJ?íD1•Úì?°Å
æ_3FGL J1815.1+5919@VÛ"Ðå`@; ¢G'ÝÀ:þ—J4À;Ñ-åìXƒ?î6,óå@ÃQžƒ8Y@‡ÿž[J¿å¾rMi.¿éWȄÏÄ4¿êTq£J6I¿ïý›¢ÄvÎUNASNone?ïE+>6É?šFÖ©¼ó†?ˆxF¹éÊÊ?‰GyKP¿?†<é¸r?"¾Oìy#?äÜ›ôŠ?Åô"Ú­-×?ÒP•š"6â?ÃéüX£àR?¯»Il§Ê?­F"÷²Ïâ?ì¢Üf|Ã?§x'?±‡ã£?žYseá?­ØÂs~í¶?šU˅tÉ9?Ý`΍ì÷e?ºTåú®K—?ÜíKk*ö?»ÎàJzª?¶Ç™šŸv?ªðӆNÞ»3FGL J1816.0-6407@t¥e¶™…À4"ÕA"ÈÀ9r"#—µÀ;¤mµ@æ?æféšõ@~6QJËU@UŽ >¹Ï¿ã©WD_€n¿æX\ãZØ¿¿æÏÜ°´W$¿ïÿ:g|]kUNASNone?ìSP=˘0?º÷¤š¡w—?³>¸
:?¶€/$I?£¬€Öbˆ?¦Té C2?ÞRØûÀÞ?ƓjG˜b¹?ÕdðÓNÄ?Ä݈XcV?ȑä¨à¼?»ïV©´j?ë²íuÿ›?§`4>70¿?² Â¾	Â
?žÍ¼0-æT?¯¨ŒŒ'D?˜°4'OEò?àÿøôX—{?¹&2‰&õà?ÒÑ-!š?¸=!Íð?ÇáôŒC^ç?±¡_Ô83FGL J1816.2-2726@ŒS£C^À€`îWaÀ9Û6òÛÀ:òyùK?ÀõßÐyn@ý¾ž
ío@aHu«ÿ¿çv¶ÑÉó¿æÙ;®_ù¿Þ™±¾Jö¿íLøÿZ¾'UNASNone?Øě'<G?ÊǛ'Âì©?³ŽUœÈ?²'žÖl£	?á+çšîC}?̄ÛÙËBb?á™õßö?ÊÁ*‰0,¹?·©íóùm?±ùey²àÁ?×ã{‰Aº?ÇAóÀ³?ہ}zƒ£B?¾aaÔÄ!?ÂT¾ç ²Í?§ð.Ìçt?ÛT#¬X?¿dc0%=?âÿdSj""?¶ÝiÿPâµ?¹L7mÏ?'L	…	C?Ø%¦tgü?·PUyXL3FGL J1816.5-1145@2}	¾º@ŽœæU4À8x‰žyÓ+À9ùÛån"B¿ðfÅê/‰0@8Lø1@Øbà¿ã¨ÝF‰¿ç¿©ò	ûµ¿émwâß¿âaÚK̘[UNASNone	?µíÍ/!?¶Þi"2â©?±h_Õq?·E½º
Ú½?ë1"E®"Î?Â_ò!mjÒ?à½nýƒûõ?Ö@چqI?•5ØÅ,–î?¢Ù(É%¯B?Ý1Äx¥>§?ՆˆX…®?ʕO_ô
?±Õ(Š?Ʋ‡f3ٍ?²}rÊN?ã®
Nv<?·YŽ=pœ?Ý K^Œ1~?ÊÍY‹¯ú´?PAHàŽ2«?V!œÑŠë?á'¹¬I '?ÊÎ\æ[3FGL J1817.3-3033?ÿÙÞ7X\À+àÞ҈ÎÀ9ÍâÀTÀ;+	¾º?½Åƒö;±@'mÖÈ#E@v?@\¼o¿ãª"
õZ¿èStM9ſ冕l¿ããPM[Ž­UNASNone?힀QGS?³ ès«7?mü|c%Æ?qö®·½ý™?²"R¬:?²½ØÙ´'?íØ^ÝÂø ?²
êÎq‹ø?Ö	~Ý%?‰ª:Àãž?®QšY?°?µ	mb¾?íœSÏU€È?ŸüÉ~²Nì?"	x"_•?"|"•YȪ?¬6Èx(ð?šŽ"¦fI?ì/©="?¦Š&†íj?gîj™?eWGŸ{?½ÃE•þƒ×?¦.©ÄGË)3FGL J1817.7+2530@Jh'¾‹Áj@2Ma€M˜9À9ï6¥®zÒÀ;Œo[Ømë?èä¥c§DR@•·+о@¶Ÿ¤n¿Ý3X$·Íë¿êù^QÊ¿âoµÅý®J¿ïÿµš1DUNASNone?Sξ?‰ÁðR>t.?h9üˆ"vß?gwØÄș"?ƒ¾Èç2¶?‡ÏÆ®kdV?ë܍ƒ"æS?¶ƒQSږw?µH'÷'í?®J/±p|#?§§§âví?¨áVTɄ:?ìÛéBâÁ?¡ÿ+•E?¨Ü'ŽÐ«-?•ÂÝPCþB?©rþÝ(Ï?–kJ":'r?æ¶Ó%Ûª?µÝHôKiO?ÂYãá}g+?±bogPX?Å_@Ñë*/?­¾¶‰	a3FGL J1818.5+1320@D§¨ÖM@*|õn¬†À:&ÕÖ`ÊEÀ;Œ¥ÉRÄÉ?ëòm–¾@æÚâå@Š`@²x¿éžˆ‹v¸¿¸×mÌ ª¿â¬"ÀcT¿è'¹ø‰¿UNASNone?íˆ/M{÷?¶ë†Zò|u? îM‰ÜåÇ?¤çç(B0?¦Ž½¤[ZÌ?²TÒÇ?æV#QO̬?ÉÓLצ—¡?Æ18Š!Ãm?ÁKæóu`?Àv:0Ÿ	ã?À9§°çH?ìîŸmc<Ñ?¤"ÍӆB?¥Ûâ½Åû¤?–Ö8*ݑ?«:&l7G?™5`´èøÃ?ãus²^m?¹Ù1×s	‰?Ñ	B$¯Â?¹\~d¬‡R?À,²>JÊ?ª³l‰×$3FGL J1819.5-2045c@%ˊ~s£fÀ"Í*1,À8÷þ×0À:‡Û…Í3ûÀeVWz?@qÛøòÆ@¥"úI¿ço-5B¿êåCÔɤ¿àLyõܲë¿æVÈ¥1
¥UNASNone(?ØìP?ôá?Íä$Çx3™?kÑ<'?"TÓoÎÉA?ãD(›bK?Î á]dúÖ?êäuu\S?ѵ -?|Ê(uF†š?œ˜-Ð
w?ÇØæåz?Ñ[í{̉è?ÖÊtÔßÁÑ?¸ûNõ>g?·¾à¦×Òu?¢w+`Á?á¢é€µ$É?¹‹ÜDx˜?îQŠõ­?3?°'£øqNÛ>Ên–è6>÷Û.c{?ªææêÓñ+?°'m^ª¥=3FGL J1819.5-1345@1mÁ¤zž?ä©À°ñÀ7éÞ(>ãkÀ9Ù)Š=D¿óÐý8zoÞ@jÔÙ`®ì@Ò$ ›«î¿ãŸ"›
jª¿ëCS‡ªó¿äêžB²¿é«F{©3UNASNone	?*>ϛð?¢EOr ú½?v±JyõØ×?‰IƒD%ÌÁ?îéKt4Ë?¤üNK=?ÎÖ*Ež"?Òs"hÐêt?"Scc? υ÷ÒU?ç§Üᒟ{?Òy=hù;?Ã	Wžv]?¬¥!í]z?À.°§iPÄ?§ÐWëú@ñ?ç1ý?²C¦%õ;œ?à¨5…"?ÊÌע Q?9tàÒQ8?CÝ$Â~j?Þ©8¨ÕQ?ÊįþgýÆ3FGL J1820.3-1529c@/Nñw§Š¿Õê'nQí3À8>ö%‹ªÄÀ9z«Yµ}ü¿ý%1¸^Ö¥@uÌKȀb@¥5À9ü¿èˆÑ§ÊVG¿é-XQ¿âA¥WÏ¿ìH	èrUïUNASNone0?¤¥íöÖ®s?¬'É×ξé?µÜy†òP?ÀxB‡"?ëúï´S.?Ãú¨ M,?à2±ºÍ`?ؒÃp4?–öÇÿ¾??¦&O´=€ð?Þ0½
i\?Ø*4Y·šž?÷J‰ù?¨õY®°Ã©?ÊÀæJF¹2?¬]kݨø?ä«ÈšËÓs?±ƒš|ùk?Ñ\ÞÕ¢?Ð9¬Y8¥?4Çîuñ²X?F+Җë}?çn8'Æ´y?Ð;Ž´ÅËã3FGL J1820.4-3217?ç•3­ÁÀ TMryšÀ9^ê䭔À;2;Yrb?ó/ÂÖ(ì@«©Ô¥3V@À]€c½•¿Ü]©¡³Í¿ã˒ìgƒ¿æ·°ÌC¿ïÿfh¥ìõUNASNone?ºi³¬ü"?´G
N'o5?àÎ÷¢nò	?ËÆå|0?×ÇɎ6ÜÉ?Éуèøhî?º(†¸ïÏß?¾AÍìÁÅu?ÝmýRµç'?ƾÅö'/?Üàÿ$u?Ç`ùž'?Ô0¤œó#ç?´'çS?ßjòLùÛ{?µáÎ2]wñ?ÈÈÒ,&9?ªyGÜÑÿŸ?Í=¹=j?ªêszÉIŒ?àôº;`?¶j‡;"`>?Ñ3÷¯?ê‹?°RØx»3FGL J1821.6-1436c@0'j¨ëF5¿É'îz°À7ÕõŒ·_À9±Ããïÿ?ì‡õÁþ)@í{µƒ@S<À¥¢?ïõŠZCÝ¿âU¤Ÿ‡d¿âý5ò°P¿ä_æãUNASNone ?ŽÒNÛ¾Á?"VR±6-?Ázü¾ê?ĨVL}Κ?ë$×"Öƒ?ńš·õ Ò?š³Åm"Ý%?­F"~ÏÝ?¸0øÂ8¥ò?¼Ž\¾Zޟ?ì$B¼LDY?Ádüî_‰z?¬÷ÿ…‰C
?™'4:¾®Þ?¼)'6å%h?§â'Õm86?ê«MàÊÇ"?«úAE n?ªƒdzÆ-?ªnx²µ°?§‡a"—?¢¬Œ¤?ìæ" ä?²Â'ۄ3FGL J1821.9+6636@X"LƒfQn@;£ŒSâÖÀ:rˆšmÔðÀ<Iqc?äEO¶²ÀB@ð`™ËX@S—Á¼M¿ëóL´ÓK¿ßuÖ¤o"¿Ûô¹"'¢¿Û
`ߌUNASNone?ïìFb0\­?jJÔ³ä•q?]‹ÐÝ-ic?hè‰rÙ&?CÎՄ2y2?A ˆrMÁ?î«·Û[?¦Ã?
ÏëÛ?™-;¨3¤¶?ŸÊAmÇÛb?'[Èìkid?–RT´Y?ï/µŽ²?"ÍÌôSö?†«ëÓ[¥?øÁM
ª?fÒ÷·Ÿ?uoÎözÄ
?íïw…x]d?£½ž9|V?šZÂ:â#?1ÉsG?£Û&‹	&®?˜\™gíF§3FGL J1823.2-4722@u°í(ŒçÀ.R‡;©À:И3hÀ;ŸÁ}ä1m?ô)Óݍ9@¬4VHáñ@TÿÀ,³?毐c1u¿Ìŀlßk¿áq™ô™€«¿ïÿô›.*qUNASNone?ØEÛgó6/?ÐË7Í¿å?ÝVWÀ-«º?Ñ.üy¥«S?ÄǙ¯¾<,?ĺOJ÷?«ÑÑ"d.z?µ­·Á–Ã?ê^1Dï¸?ÀÂ>°0"Ë?¿%Nžk?·Ûɧܪ?Ì
Ì»Â:m?²'Tí­ ?ãjaËtt?¸¡ûÞÇr>?ÆJ½óÅ?²Xºwl6G?¿Iœê¹~T?¯å¡ÑUþ?éD!X]?¹Z«¦hùR?¸v ô;¾Ã?ª–Rþ3"3FGL J1824.2-5427@uE	k¹Œ~À2
cÇOµÀ:WL0À;¯rçԐ?éƸ	µû@}ò

@¥ØߪŸü¿ãYÝUtëS?®ì:•ñý¿å8S¦ù²¿í"vmUNASNone?â–WA|m"?ÈÜý!\í?ÒSĤ§˜ü?Æ!÷ƒLÒ^?Àÿ°¿?À«¯ª"&¸?ä¡4SN^5?ÉN³‹—¤a?Ë4!?C?ÁëÊǞª?ÂG
sƒx?»0-¥¤¡?æáã"a{?³Ü—û Û?ÉՎÁhì'?¯îâNŸœ"?»eÓd?¥´´£QþG?â¦
—vF?·ú·$~l?Õ¬ R»Ž?·Â>€¤¯Ð?´ÿ]_ž?¢Õ½ÈÌ#3FGL J1824.3-0620@82Ø]ú‡@©U´g{9À8‹'®›‰^À:š'Bdÿ^¿õù}d¯­@
éGZÝq5@òø‹áu¿ë(¡–­¿áҝç˜;¿ÊwÃÛâi¿ìè2a"³UNASNone?Óóòc*Æ7?ÈÛ¶;´ ?Ӌ?,·Dž?ÉVÃGøáÁ?؀Îpõ*?Ëz5z €ì?ç¿MX¨?сõK°a!?"c¿cªc1?¡÷(7N'?Η'–UPþ?Э>–wÑ?ÔuM4'h?³ÑkÉ$¤ù?Ψ"K.?¯ÊÙZmj´?Üù6¡¥Ö—?µÔqqÛâ}?惋$ru?Å!{ÜðJ?Z]z¹â°Ò?jõ­°‡?Òތ=8e?Å'Ҙ"7¸3FGL J1827.6-0846@6k"Àh¡?óݑ[¶ÓÀ868À:;¾íæù?֘nyé@I—M¹ò@åÎ 3ý¿çAT惤‡¿ã²')Þu¿å·x®¬?'¿ççÁH›`UNASNone? §.&ú;?¢¢dq?¸öÌmmg?½&ѦÀns?ëÖ³ò0P?ÀÂÀÓø˜?̅a:ñ¼?ËcFn҉.?²…-¾ÄF?²'²qÁî?æžw‹¸T?ÌÑpïiŒ?ÅŲyA›!?®"7³î—w?Ë|ŽjŠ×?²~Ö|íâ?㯋þöƒ?¶ë½·²?Îˬ×äã(?¿¶:›}[?¡Gà|+Z?'ø°TãH?ç8¢ëÿ?À{ŸÐ3FGL J1827.7+1141@Dd	þ†ƒ<@%	Ž«ÿÎÀ9›iK4ÄÀ;[ C×Æ%?õe3€µòì@
9r&@år?ãoÑ?î4~{ŸÍT¿áp$2íÆ ¿áOþðáT¿ïÿð	V¯©UNASNone?·oùw¿e?¼"UL?ç¿Í¦Íá?Éîó÷?ÅHÌ«Ñú?Æ®Å`¬Ë0?˜jcÙ<kÛ?£÷ǂSĔ?ëa"V=?Ày%e|'‡?À¶>O'?¿´TÄ È?ÅIû½í3?­:Š½ ¸´?åºoñ¦\?´Â»#ÀŠm?ÃÌE¨¢'?ªÚމ ?´
Hx±Þ?§{YÕ©‰¼?èž÷'ùr?¾ÁÈÎÍ?ÃÓ§ÁK?¶¿oÀ¿¼3FGL J1829.2+3229@NRs×Ûõ@2"Ø#B$hÀ9þJÁÅ1ÎÀ;¯Ux™]?ô)ÎØÀ ï@•kâ@H?ìT'?†F¦¿Ýl0%Ú'¿çÈRoò¿ïÿÆ:Gµ²UNASNone?Œ º¢?ÁÈâ%æ×D?ê¤;wÉ?Ã~"ÀB?'zxJÀ)î?œ}íÓºL?ÏïTáyšH?ì­'w6‰?å¡1¼?ĵ­\¶$?·"L´Vëb?´6x3?ÑÕ9b@ç?¶CLTvx?ãF"\]?¸¿‹Å_E?¾v"þlR?§M
jÞ¢¢?ʧÌõÆy?²\»|Š¬?ç
<ܦM¸?·.‡&"Œ?²^âK?£ŽïW.µè3FGL J1829.2+2731@Kæe+ÓÃ@0­Å÷Æu›À9lg"cϳÀ;Š¦Bˆ?ðÊÅ~#òN@'‡µÁms@õЀ5šl¿ãÇa/Åæ¿êbà[09¿è'íþÔ:¿ïýó®Á|•UNASNone?í;Q$Fóü?´8úUâH?¤ö'¼¦lƒ?¢¬»ñy˜R?§T[þêSÄ?°],Úª?ä¿!äØ &?ēŶN¼ö?ϸe¡vØ?¿ÒËrp·†?º–%—"?·éš
³ò?鍉Þ<L?±àjéû??À–A5ZÌ.?ª£3É"?²g.£iÝI?ž›s\B"M?ށÛôïB?³ó7‰;.¨?×à å€•Ü?µ9»}Iu•?Ã;K¹Ã?°ÆËCâ3FGL J1829.2-1504@1ÉêpLÀ`QyoW§À9$¤úö¬À:ºÊ9t•Ô?íE!@R¼¢@PԃÐZ?ù±Iß/¶¿ï\ ރ׿Ç2"J¹¿Þ†$æÙR¿Ì­ÞJÄUNASNone?âÛ¼ܟÚ?ËY¤f×d§?²SX;È(?²:ߒŠ.?Õ³±çƒÎC?Êâ¯Ù?×Ð+X˜í?Ó*¿î3‹ö?´$6Šû¼?¹3y,îVH?á"c'oéº?Òc°fGA¸?áŽÈ_a?·¢ª‹‰ƒS?»)!å¶SX?¤ÂãáÝG?Ö§G¬f?¶TÙòÖ¯,?ãÉ|ck?ǁüŸ|N?›F8¸6Mb?£ßtiþ?Ø$	{µÄð?ÇFÌ88²§3FGL J1829.3-0135c@<ýæ>Ž@ÀgHäu`À8É2=jÀ:hƒwe?áŸ4eã3Á@
¨×z$ß@JMà]£I¿Ñ-ðŽHÌ¿ä¹ï[ ˜¿ãWìEÒ·¿æ¿ÿL¯c¹UNASNone4?qD/	ÞÅ?xvÔZŸÚ?Ÿúxä}'?¨{"›+QØ?îÝ£Ú³ÿ²?©¾Z²
CU?éþ} u,N?Ä&ižU>z?›è2±? ýãý??ĉW鸣?±‰¶ )?͖i=™)?±XÎ"³?½ÛðI+ú?¥ï¯â2¦m?äÞç­P"6?³RT!N`í?Å2éû¤?Àmy—¤é¥?°¨^&?'ï£ð'<d?éÑx³
'?Á\n/QAŒ3FGL J1829.9-0203c@<¥£Â‡è@°ò¿-¨À8~MZü¦À9åÈÂ|ó?è˜è…K?*@©ˆGØ%@åŸ×vI?ì\±àüôL¿áJ~]ö+¿áBö\"(ç¿ìyI{…B±UNASNone ?~Ë<f¡?"ÊÖ²F
Ú?áÁ»|‡:—?Ñlì¶Q6p?Ü\YN?ÑpQH3Íd?փH´€>?Ϥ9fXۏ?эVs=³Á?Ç>Î%1m?×ï`Ø2Ì?Í· ÍÊf¦?Â¥4[x˳?¨¹ÑØÛ`–?ÔЊϚv?±Ö[T¥©‰?àô꣹ÿØ?²Ã*ºÑ?£æò‡;IJ?¥ê?,‡?ÁX£@ê"%?¹œbiÕÛ?êkhQ¦b?¿‰ÛïÎ1Z3FGL J1830.7-1630@/Ò¬Ùè>BÀ=Šú`"À87 ޜØéÀ:‡ºÿDï¿ÿ˜!<Ю@"ˑ¹Pn@ƒ>@'|¿éôÉwq•]¿âa¨ÀÂÂ!¿ãèH¿?#4¿è€¾­`‡UNASNone?ã­lfR?ɶ•EÔ4?¸,kQ7?·ëÝ9µL²?Қo-±|?ÉúL¶?ë>j¼zȟ?ÌR>ûvƒ`?•é]Aé?¥¹[]?Á,öxC©f?Ê´ÔÛgû‡?Öh'!t`?¶·Y­ËÊ?Ç]Jÿ'×Z?«°õ{ÈÌ?Ýé3^´B?µ¸ìJ‹z?æùÛ$PÈ-?ÅkI=­õ?[&lráV"?pïjϗ_?Ññ#JëŽQ?Åfw.œŽ3FGL J1830.8-3136@՝CrFÀ#®ç£è`À9·ÙfhÀ;TæØÍ®?ìCÓU–Ï)@
®ññÊ]1@€®_ybB¿ßu¥Ô:X¿¿³ý!£ê¿æ+x±Â…K¿ì8BáòUNASNone?³GHÇwëò?±xþúޚ
?åõàfj?ËNµpSÈ¿?Ñ$âa8-?Èp[æ±ßB?Ò¢|‡§Ó?ÊÍÞ§Êl?Ö©Caµ§"?žéMèú?Ö´­!°™?Ǩ®·†a9?à/ØÅð›?µhŒé¼ý?ÓßCƒ"?±í€î3á¤?ǂfë7O?«ž²œi…ß?Ô{Œˆ™7?³?ÉO'o?à©ó–'—?¸¦XÁ!?ÆÃ-"Ã5?¯¤ºa"]3FGL J1831.7-0157c@<ðÞÁÁÖÐ@źcdÀ8U["¤À9›hýð[GÀ6O†{×@
#nýcÃt@Q¿Š¿ã%ïÓ·ø¿ìxÌwí\¿áœºBÜs‰¿ã–σ$UNASNone0?¿0 Ù^?"üö/{?vW7J.M¶?'•ñ5Gé?ï"Ó1)ð¨?Ÿ½7‡—¢¨?ë5ÙAf¸$?Ï£¡u»p«?}ì||:NÍ?"ïՒ"á?Â97ƒLü?ÎëHêZøq?È´É'+X?±í:Ý?¸·Ž,€€ ?£µêÉw¢?æçae?³¬­Xzä¶?ÖLüt!ã?ЧîÔOþf?oǪto? À®S÷Ñ?äÙOƒˆ›n?ШA¼¢­13FGL J1834.8-0630c@9?î¢	ª¤?ænø`¤Z"À8í^<Ì9À9Øî
5?Ñ𢐟[6@¬fjÃl@²m?ôa¼?ë S0ºÄ¿íö:"`L¿Ô=XRHï¿ÛóÜApUNASNone ?úª'¯¾V?›Ý''øÊ?`M¢"Ôr×?wӓq?ï§Ç³'l"?žÖK§Ò®?£3%F#øo?¸ŽK^RÎ?™ ~n×,?£ß)µc£Í?îɸ'?¼+™+?Èspànr«?°êþo×Ä6?²ùü+»Êm?¡'."àÂ?çƒäBlê?²"¿ºš{›?ÄÑ}ý‡¾?Âb¡}§È?b+Æ-œ?p	ê?úâ?ê¹tºq?†®Tg')3FGL J1837.3-2403@#±©É'†À<µ]D~µÀ9v"´/GÀ;}}?ÕÏ\t@9muÏ:@6tªL¿çá©	=\¿Ü,Ûàæà¿ãQG¯'[ ¿ï}§SÒ¡3UNASNone?ÑÌS]Ù?Åbs.è"?Ü|¦ÂÿÙ?Ì\n´p=E?Ñ·Ÿÿ–O?Æ»7xk\?á[47ÕVð?Î1=|…L?ČoÕ:^w?½\³îóà?Ó_¥¸"å?Ç­î™øŸ?â˜ä"ǐ?¶Ò	¼ºH?Ð5=vQjh?³[a*z®?Å1òÂÞð?¬Ž]@V?àZ!†ËƟ?ºWoðùVÑ?ÃE°gvµª?²Lf±Μ?ը侭î?¹Ý§rÒô3FGL J1837.6-0717@8ÝÔÇm{¿Ñ0‡¼øCsÀ8Y­N'DÀ9¹÷[ÐL¿ÐÈlåJ`æ@
Âp¡æð@L¶€… '¿ìpÑVýÆ¿Ìö%°,œÛ¿çÓV˂Žª¿ãËy:{žUNASNone?¨UA·õc-?¯ê|èËM?ºw'ÁòÊF?À• %ÒÕ?ë+¹ŒBP…?Å0Ž?Á®¯[®R?ʔzÚ?¬ZqÅ
µ?³üЫ¼Ø?éέÒ~?̦ÜÂùA?ÄKVCîN2?­,Çöq?ÍnaMIO?µÊŒÖĆÕ?㑪V±!?¹:Aî=?Ï˂1+n?Ê+%pLÒE?`|"Ëëb?ƒbŠ‡|?çǝaôÍ?Êvׯ+;Î3FGL J1838.1+3827@PΚ¿3‡@2åxåÄëWÀ9Ù ~(ØÀ;˯é(¿èCc˜D@›@ññP@̾@Bo¿é‡ŸeØÄI¿å;qv¡U¿æ¹˜ÿ"žÏ¿ìÍÈl¸2UNASNone?î¹îŽ/íD?¤4m
БÜ?"¯3.Ìm?"'r ^
?•û+Ӌ?P"4µ?ï
.pu)½?fÌ!qÊ-?‹,@	3?ŠÐü¯r¶?'4›ÑZCÁ?•´`QƒÙ'?ìÞùÁ®F?£*å÷!D2?¥ñSx˜?"~(˜k°ä?¬OÓ˃?š-§Êîœ?îLз¡ä? Îå	"¢?‹Î+iêÈ?Œ8täI•û?§'¨A§?šKOÃ3FGL J1838.9-0646@9zTæâ!É¿ÔAKdWmzÀ8:úêíIDÀ9ýèwM>?ÓS–=w7x@RQR-q?þ¿>«Œ`?îÅUÌ)'°?ëL¦*õÏ¿ßÙî7D¿åŠ¯nÍ#UNASNone?"W¬.Tœ?–Ÿè$ò0?ˆ%`°	Ó?'BJv~à?îûíÍ4?¡4›ßÓU?»‹yƝa'?ÉtgôÇ^Š?ÅJá»øÐB?ÈàMæáå%?ç;ØX.Ë?Ñ\ûn&(é?¿í£i]Mc?©ø‰"ú?°#<ÃTV%?^mœE?éýãúiˏ?®ì"¤¡æ?ÐòŒ¯m?Æ/6úï?Кª…¿éD?Ë)íÐç³?Þ¡'dzgO?Î=÷þ,W3FGL J1839.9+7646@[8›R~@;ÅïbúÀ:po»y¾2À;ÿPïܹ¿Ÿ9%ÑÐá'@
˜áT@ld¿ó¿ã±Š#"ê`¿è¿|¤¶¿âܪ̃¿ï"wõºUNASNone?îºÊTÅô?°9Ï^·B?'-©pu‡?'(ö®¥y?©¸èþ–>÷?­Øa2¤Ÿ?í¿þ¦š6˜?¨Å~)‡˜Ï?§Î0€K? ôzŒÐã?™ÐŽË¸—?ší¾(ï?ìµb€–¦?£*]à?¦ÚÈMuõ?"x>+§¶?®Šù©¢?›{Ò`?ìë˜+,1?¤øRs%¿¸?¥´æÕâ?˜èf^¢µÇ?«'–wZר?25iÆX…3FGL J1840.5+6116@VÀŸ±@8ÙìÔªàÀ9Üuι6À;›¤xð­¿èù+¥þµ[@´D¼­@۞ÿµ¿ë÷&~*8Ÿ¿æ:QB›c§¿á@Æ®-X¿ìªJkßUNASNone?ïÓOü/Í?‡ÝîbÜ?eåRØP¶?j.ą}"?fÊé~
âÁ?vÚÞGj;?ï‹Cߥ'á?Ø&á }å?z?žVq«?€s6¬¤ß?€8ëbr2?"'3S¹?íÐ¥nØq?œ'Üsáª?œ>™†'¸¶?‹X*2
?¤Ö\O/'?•%ëÁs¡+?î·]ï_O?•ñIöîæ?hÐb9ñƒ?gãöΡ´?¢ýæ~¼?"ø1Ɉý3FGL J1842.2+2742@LÌݓÄn@,18yÄ<À9'íG–—‡À;|5vÚQñ?ìpRqx#Ž@
?çݟX@!¿mh¹¿ãMû
Qø¿ÖŒtšUè¿ßGDŒ¿ëÙ<\QºˆUNASNone?Ð^f}N™"?Ã9$Ù$[–?ã
ƒ?ÇiDÁì?Ã,Å–Ï?½$^ðš]?Ûaª¸Ú?Ç»C$Xoµ?Ùb·£g
¸?Ć]i@
A?ÆxcexÛ?ÁÆÓ­'l?ãÄÛ筞?´]ËüãñÑ?ÐLÅj²ÄÅ?°Ò<2p?ÀSöû¿ÿ?¤ý	ֈÙ~?àÔ9ËÎ?µºS)ñ[¨?ÕdêÃQ ?·€›<¢Õ³?ŹåCk-‰?¬'a˘ 3FGL J1844.7-1224@56q¬À¦žË1ÂÀ9Lx䓓À:›¸®ã®¿ÖYIŸ}«Ÿ@­5'Þê\@9*Ÿ»Ç—¿ée÷"þW½¿è·×À⯿Դûï=ÿ¯¿áŒë¨ÛUNASNone?ç >D{?Ȃ¥²èýÞ?ƒ>Yjüôn?‡Ûy|6E?Ð%'2ug?ȉ9™õÊ?ìéÈìG+?¾NO¹/r?âÁÎΠ?‹"ñT#?¶ugXcìÒ?¼ƒÛ[Çï(?à&zX)y¾?·r=Aùt'?µîsÏ?£ÛfÁ?Ú7nŽ¬GŽ?¶T¢þÈ?é Š¤´?½êoÝòh?8jþȼ×?=W~{ÎvÞ?Ës¨VY#?½äÒ빇3FGL J1845.5-2524@"á˜kœ0MÀ$(^ÃÚµÄÀ9]ÉòîÀ;*¾áQ¿?äkõö«‡G@
™•}U@N@A0ÿÒ2½¿ã©åÇù¿ç¢I-ÆaÏ¿Ö'ˆvîÀ¿îIt&(ÄÖUNASNone?×¼Êɜ?ËÆ&Yߥ?É?vâª:T?Äü.@Æð?Û£ÂĘ9?Ì'Ãbíu?Õ¯0=Õr?Í"8Üf+?ÔoúÏê‰H?Åá)'|^?ÕàÔò@š?ÇÔØKüfã?âaM¯ÿ×Ù?³I$ª,Y?È·†«O^?«žÀí³
y?ÍÃB"íQA?®­çhö]|?Ú)mj¸ªÔ?º9¼3$¿?ÀjZ%å?µÞY~Ú&?Ý¡eF´Ç:?¼âF
Sr 3FGL J1849.5-0124c@?v«%(®¿ÍÇø<<FWÀ8Ê<ϔ'À9}⊤3Q?ñÂãoPšÍ@ÕÅ©@Dàßÿ.Ÿ¿æ•H\mÇ·¿â‹ƒ&´(¿æÌdÌL8,¿ìFeXäUNASNone<?_ù_í€m?`âËOÍþ?äïW‡–Õ?џþU…"Æ?ÖWäÕg?ќÄe'F@?‹@»TRs? `@udvc?Ӆ\¤Ø¯Á?ˆÛùSò?åÐNÁRVÖ?Ìa¾Â@ލ?¬äuæÔ?—\Oí­Ž?ÜÎüñ	î?¸]Âhq?ß°&€9Oô?·¿bi~é¥?ˆŸrG·¤?¥ ÕM±'"?·fx÷u?±Çr-jð?ì&øÞ£T?¹Û:6Ún3FGL J1850.5-0024@@;ò<ÈÞ+?'çT¸i"À7"ºV¨ƒÀ9¦AÂB/O?ôÇW<§Ñ@¦ûjo	£@[?²r"¿Øò‹p¿ŽS¿é™Óêè¿æ†Œµõ3¸¿çÍ`|Ü8iUNASNone?rÂúxkÒ?t{öycy?¨©/Ÿ&¼?µ#fùó?îOçì¼?µ¥»/i?'mSYB?žþ"NS?µ­~HÖ?³P΢°Ñz?ì¹bEœœ?µÖdÈØy??°,Uj®?œè9ä©VS?ÇÃg`¿[$?±}­´¿
?èd"E{á?³r£Cuë?±¤4zr?®nW,?¦Œ5à!"?œBƒ)(<?ìzÒ¶  ?²©¢o;ƒg3FGL J1852.8+0158@Alk΅3±?âЀÉ"À77ûº !ÞÀ9Ã~ü_a?òýó¦*v¡@üäõ‹C@`Пëf¿å0ù›ü!¿ê;ƒ[6)¿å²Æç'¿é¬ƒIS¹™UNASNone?'°NËÌÇç?…® ä†=?£È)D?ÄI"
µcæ?ë0UÒÌB?ÄØÖr/Ï×?"¹xr«¥7?­±éñȬ?ѝïëJ?Áe#h )C?êLÀ¦h?Ìl6Ë©?±êvøÚ¶?Ÿ| ¡ è;?Ñì·	XlW?¶Z^öùìÀ?äÌUœS®}?¸2c!IP"?¢žfµ~"? H(4b"…?¸Vt"Ê:?¨

x
5Æ?ëËKu…/?±ç­:u\m3FGL J1855.4+0454@Bá
£3v?õ¥+•°À7ÐÌ% †À9ù¡t?íZªŠF"@
:íO¤-@W— mˆÅ¿àï6ð3À¿épJÜ$â¿çNéWпèržïïUNASNone?pe¨
ӌ?uŒç\‹¾?ÀÛµ(cöû?ÄdæGÍßÐ?ë§óê–ìš?Ä wÅhí?¹óÆÀ«p²?Ä.ù×ÏW?Êènnª?Äõ÷¡sá?æ&Žö??˸ìa~é?º~Ž
‡x?£¢Qï´?Ϲprm*¥?´2æSŽ¾?äÁ´£dh?´®éE4L?¨§ rL{Í?£fˆÌq¹Â?»lÎÇÚ¼=?­;‰5³Ð?ëôßà»?´ì~Éx¹Í3FGL J1855.6+0753@D7Æø@B‹`òËÀ8J¡!À:^×òš¼¯?êSrBèˆ@xrÊø·6@Њ©³¿æÚ¯Nњ¿é
X<Ï`¿ãŒ˜qGã;¿ïæ_4eYÃUNASNone	?ìg:ÈCª?Áê#d™?ϲ珎È?ÌÒæ…t!%?ã(,MjJä?Ð×f%˝M?˜	<`BQ?²î§»ª•?䕻€¯?˖¯ËéÅ?ÕSö
îÝ?ʈõ™²&§?ÅÚ.¼IÏ?¯)ÿ"y?Ð'àHg&?²½L '?âuíD,¹ú?·ì¯Ym?›‰W'ˆX?"Ј¤3…¹?ظký?ÄÚ¶˜5kÄ?ãYEm5?Åls¾‰PÞ3FGL J1856.1-1217@6whۋ¬Àf•Ù¸éÀ8î¾c}}ÚÀ:ë´¬D—	?ë«Ë<vJW@ofw®7`@¶?wå¿åíQŠ"̉¿ë7ú&ïzn¿ã€<"Åý¦¿Óm'ÔUNASNone?ækµD?ɊԲ^þ¬?‹Qù¾}6?Øœ?ÒOj*†¬ù?Éx˜Ï×@[?éíœÉ§¿Œ?Æ*Ït9LE?ÔDAB(?¥ŠÂè}w?ď
°Øً?'#-ÊNî?å•·¢‰‹?·—èá­ÒÇ?³nIDý›?ž?KW´¬?ÑM¾i­ƒ?µrfè½ò?åÆ
¥.Ä?»ÉðÎí?'÷NÏÛ?˜
ʾ±õ¦?ÓTs½ŠÉ?ºÖɶ9+t3FGL J1857.0-7341@t]9–ûÀ:W/˜sÿ¬À9¦ÃhŸýÀ;¢«%³ð¿ÌÙÑò?fâ@OüÄâ@;z¿ä±ñ¿é€ê&¶v¿élᄌ8ª¿ç؆ð'M¿ïÿaXNeUNASNone?ïÈKæ˜?z²ô"IO?_l]Ʀ)z?cø×F(?tC
ã*^?u—iôqõÿ?íÐ=§#†?°Ò0·ž?•ù¬Õ'z?š$i3Gé?§ÿ˜·\Õí?©—!ÛY¸?í‡]!_"?›2ˆÔXY?¢ÔÌYA…?9Šš"rH?¤µa•Øˆa?'–ÙQ,?ëN‡"¯Íì?­ë]üˆÝ~? V^ý¢÷?™?_ìOR?½`»»¿#?ªfH6ÒÐS3FGL J1857.8+0129c@A€jüοè	_s­øÀ8+-ß6[ÝÀ9t°/Þ?òö&Û6@
ÌûìJ£@½Óà'Q|¿b7ž¤&ƒ¿ç¡YMp™¿çÛَÀçU¿ë9ì¡î·UNASNone8?NI|)5?Ru"^?Ò`"K ôû?Ж­`4ïF?æÈ$ay?КÎjôï?¢ËçMí/?²eŸÊhò½?Òµ"ŽwÇ?ÉÞÚ¦Ÿ?åÆt§ÃåJ?˺¿gø¡&?¨u–BQ,?"í~úu?ÔR8£uaÌ?´—&ԏ?äUTá*?µW	.êܾ?–¯¯ŽæÃ? äÍuŽþ=?²n~úkŒ?­š¢ÿô…?ìü²§Ö:?´ÁɂÝJG3FGL J1857.9+7319@ZŽ4@9pJ¥?À	À:
ÍfOÀ2À;ö{í·( ¿ÚÇH¢õҙ@âÎ}Q@'R€«a¿è¢Ç:î¿ìzá%Qü«¿àj$׿ÑÏTŒ[áUNASNone?ï¡0'ºIç? \ª`_k-?XC¡T5Œå?j­Ž«C!þ?"«k&æԄ?ŸÄR&ÞQò?ï…Ô ñº?›0UË´ü?{"å"
?‰{ߞÚó?€ùˊú
´?'óôûZÊX?îG]»yö"?•±¯­ê›?Šåp®X¡Ù?|ü{"*?¤ÐÈÊnN?'`G£k?ïGñ¢˜ ?¦CL¾­?PÔÅñ{¬?Xå'CÚÐd?•ôlÝäH?ZÍ·(ø3FGL J1857.9+5549@Ux+Iº@5GÎÙ‡+À9Î.ümÀ;GþœR±?Òvۆƒ0@Ñoƒñfµ@°uˆ÷5¿é]h»L¿¿íŒQ=pŠ¿Ï||àØ¿Ô¼ÊJ*_iUNASNone?ïÄÖiq?"JP…Ò?PÿîSÎNš?U÷ù~cóú?yµ6|´?ƒlÔµ|u?ïw½9¬Â? ÿüô"?~®µË!4¢?' ]v‹'"?'Á5Ì5D?"T5jÐuë?í™ç T¼? ¬Í½¤?(¹›Rå‹?€ª† Mƒ¢?®M1-
Äo?œ‹åüzo?íq˜µâOO?«YÍTmF?o$ÐS?L;?|ï
"AŸ:?³zÎS‹'?ªú¸HÙn3FGL J1858.0-5423@u`¢}ŠÀ6­Î|Ð57À:&:ØC""À;·¢Ëq'ú?ésÐ#eØ@
Aå·Tj@ô<ŒAí?ØU$äTÿÜ
Öfma¿é£*—b¿×ñŒÃ%ÜUNASNone?îÍg?°îòqš$?¢'©§î€Ø?¨rØqÐûJ?—º
ŸéQh?¢Ü£.© û?î2œçÜú´?²-fÆ}?'<:pÿ7?€·Šc
?£¸:wÕ)?©©Ò"å'?ìÏ!µ˜L?¡ó'ÈçÍW?¨¿>$W\?˜¾{‹îD?ªO¯ÀOcá?"oRâáøY?è¬Ú¼#µ5?¹–ºë°[?·¨S¼áXZ?µ·÷)°=é?Áxk1?²zëñ,øƒ3FGL J1900.3+0411c@B×u}Zž²¿³'¿ž¢(EÀ8XU±ã<{À9ÈQÎÿ¬ô?♺™Cˆk@
Â/,"[è@ÆŸŽP:¿Ñ:8¦öµ¿è"[clÑ¿æö&Ó±öæ¿àK!2߄UNASNone%?dx·BK‹?i'üu[ì?"¯&E–0–?¥9¢SQ‰³?ïNÑ0?¦ÇuAw0?¡`Õ| Ð(?³3àD"'?ªo`û!?±â04¶Ñó?íI«².A¬?»´éóãÈä?º=;
ª?£ÆpRÜõ?ÀÙø_*j?ªÝªÉHâ?èÚv› %?±•F5á?À¶;X´ý?¾C©Åù7€?†•4•ªŸ?‡¼IW݃4?ëxeÓ(E?¿¿­ë´3FGL J1901.5-0126@@f…ÂL@JÀ]Ç@›Ñ'À8	ð1UãaÀ:'%ž:X?ÝÜ背'ô@fÖ
hHi@ò'ÿ¿âül`(‡¿èõÐF~êl¿æ"&Bý"¿é¢ó*ë¢6UNASNone?Ü$&÷iÑH?Ém5`¯-?±«D*ø÷?´¿[IƒF;?ߖî7‹p{?ÊO¨!
ç_?Ò2ÆLùq?Îí8ò»Æ?Ä7>n³!ç?½K…s7Â?áå—,ºÎ?Ìû™ƒ?Ôöàhç]?¶Ã±?…Ûp?È^SwTÕ?® ÛGÌÍ?ÞÚÅÛn8?·…I=ãu?փIu¢®M?³€~|M"Š?°"Vïøs? "õbcY?⻨ÚP©Ì?µ«ç¾[Ž3FGL J1902.3-3702c@v~ᛐëÀ1öwÄ\»ÃÀ9¾'²˝À;]Öì
¶?òb̓ìÜ@
ÈpëÐs @ˆ/ž‹q?ãÕG§€ÚR¿æ½@šF_,¿ç¾™è7Ñ¿ï ÖÊÛ
¶UNASNone ?Ç;ìFg?ÁN°·Ö?áwx¬÷K¶?Ìy":?Ñsen5?Ç
×À×E?ÑÿªExz?ÇÇfÌrwJ?ṝ~vø?ȀÊ~ÐTG?Ç¥Äÿ/
?½q^«ò?Ý7£0ÃÏÃ?µš\Ή{_?×2ˆîŠ ?µKáó†÷?Ç,ŒŒ›L;?¨—á9Ê?Ä×'à7°ö?¬À…ÖvD?â–{µ``þ?½À÷íýë(?Ðgt¥#eŠ?¶ÿ1;"3FGL J1902.6+0655@D/Ù<FØ,?åԄƒEÀ8‰GnSš²À:Vgâ?âà:Üä‹Ê@áÊf–@؋Ÿ…ì¿?ïý—"ìпæHXT¼2¿âoO°0M¿¿å¦ÃQqUNASNone?‰gçƼ€ö?"('Fâ;A?¥ZH?°ÇDæßÇ8?îHʸÌô(?²ìZƒûö?Ž¥.Àr¬?©°m,·?¸˜EcçË'?¾,ÆCl—?ìrb˜>E?Áאdn?¿wÑÓuÓ¼?¥Œf¾F^?¸oFٟoÇ?¡´iò«˜ú?éê]W?¬óG··ˆé?­6Š¡wî7?«djWe%?¬*?|e?¦ÞôIoæ?ìiöAø9W?µ%ìVÑ3FGL J1903.9+0052@A'ʽf'À*ï9ßßÀ9O²G^cÀ:‡Ð|"µÝÀÙchÛ
Ó@ˆí$C@'& {±¿åšxBB+¿ïÇ>㕑!?í<F'Ej¿ãÔl~XuUNASNone?Ü~lá³1?Ða£œ0¥?l2}¿€ko?r»†Qµx?á¤ÁËÏ¥ü?ÐgÀP
 Ò?é¥qÞrI?Ó°Ò
fã?~̟ämcq? óŒQŽÅ|?Èu'9bËÅ?Óc…raS?Ý:»š?·šÈ"-?²{_Büó¥?¡‰DºÖ¡x?Þ'l…)?·Û:ñå?î‡è4¤?²ùjþ˜}G>ƒ r\r©‰>²ÎhÞ?§	é`©?²ùjÑct73FGL J1904.7-0708@<>iƒQÀÒWBÜôbÀ8'
DŒ!À:ä
ƒÁ¿ý¶3@=Ä×5›@²=@RU¿èØ(Ë{>¿ã@ãëªæý¿åø|
Ë"[¿îkìï.UNASNone?ä`.¬ŠÛ?È/§îo'ç?ʔ¸«/†?Ä2|b2O¼?Ãë/•)dH?Á\ØDk²?íßy]½'?¶ÒD—nT]?ƒ}hˆ+^Ç?">º6­£÷?­/~HO)?´·Š•H?ށ+¢Ó*?¸rLŒò*?ÌE	?ù©?­äy8=̤?Ó\IXŒÙ(?¶Ë÷Œ™??ê‰kòB
?¼‡Àtl?tHžG˜Õ?‹ŸÀëd?Å9=]þ[?¼8›Øt3FGL J1904.9+0818@DîE܃#6?éẃ}™À8̀eëí$À:&h!Q‰?Äw,S½d@û‰Eû7@`<`ƒxp?ìÏ7x¾ê¿î›æË{"õ¿Êï,ÀtÇ¿Ü}ìÑ
ZUNASNone?¦˜¶óå 1?°çتzQ?u…"8áü?ƒ1\ÀC
?îkiˆQ|8?²#Á63¶?¬Û.ΌQ¼?ÀUw¾$–?"½ ÕµF?š±KÞD<­?í"dn:?ÀÕ><E/?ÏÛ>©÷²?³pŒ~TÙ3?®!Î4=a?›Õs–á?æ'ˆžÜ=?´Eçgâ&Î?Ø>¿ÆÌ?Èy‰).P~?Q—"B'õª?\z%êt¶]?ãØ+ûPƒ?ȀËñ¬-v3FGL J1908.9+1022@F©æî·?ìJ¬áõÓ×À8T=ÚV"LÀ:1@\¢?óÒ‰šs@
£'䞥@®Ñ¾¿â^ñ¥™Ø¿ç©Õ7Ä+W¿ëΐÌEò¿ßº¶L5kUNASNone?t¶¨íϤT?{Ba‰±Þ?ƒ×Dëü?Åß̐Ê?ë5œÝ %¸?Æë}\а?Äø? s?ͼ\J$?Á‡¤KÍ\?Â=™>OâB?æ`+JÍ?Њ2\ÉH£?¼{_ܟ·¥?¤›Zý€^?Ñ{+åí­?µÍ<a;?ãçVny5?¶í+ï¾4?½˜G)WºE?³ü[‡g?Â)cõêT?¿‹^5Éö³?çžZ‡#?Á[ÌG¿t¤3FGL J1911.1-5318@u{sBí»ZÀ8Jt֐›À:&ÇÚÄçÀ;¼¦Ô¿«?óŽP:U~@
hÍ°LŽy@žÙ€\¿Ó3T·xì¿èx1Ÿ+Ì.¿î~.ÔÝ¿ïþEõF'_UNASNone?âHzž™ˆ?˽òAÀ?ͲÍ]ð?Çe€ÒŠÏ?ÊÎÄb¸;ì?żU[Žƒå?ÏÍp¾?ÆÃl7^´?áv…tš?ÊΛy?ʨš¼Û?¾ŸýIZ×M?à¦Òoêh‰?´6wugïj?ԅ+Ç}>j?²Ÿw*ŽÁ?ÄZ^±[á?©\ h'Î?Äò2ßÌáŒ?²"ñcÔ?æžÝ¹—¸Å?¾N;óÏ\?À'V9Ô;^?±Ýõǒ¤3FGL J1911.7+0307@Cº`Àœ~VG4À8ö}«ýIlÀ:·Ÿíp±¿ùMÛÅãúf@Á~Ëb@"éßW=ÿ¿å&5Bpם¿êE[–¿Úx+¸ô~¿äùõ§ÓUNASNone?ä
û€Ï€?Ëtˆ»•-G?zŒîhÒ?}miq¯d4?ׁÆO]í·?ËtðÖîGe?êE<–#"¼?Ì2$¸çì?Š'òzû•ª?›	itz?ÅAÞÂ3²?Ëë4š7?àÁ±:à?»âÐÁ¨"ý?±ÓqEC¬)?œXԑ †;?ÚÁ8îìå?º‰îÞé"?첅‰–Çô?°:(Wßça?çÆïBçÃ?Rb
Z´é?ºgYÁï¨?°9"`.3FGL J1912.7+4610@SJ«Š\å´@/‹ºw_²îÀ:>´~!nÀ;Öq»g¿áŸoã×o,@.ÁÕøÅy@‰àiÝ¿è#ðÿ㭞YzxJ¿äf¨6{£K¿åðËLD&KUNASNone?ïRé[ø?¤ÔSRr'?pg·?ëGg?uÜàߤ~?'ˆæ±N#?£"¸©©u˜?ï=	»´ ó?žÛ®gL×j?x¼×©9̄?}>*±ý»?'/'Ÿn?›=‰¡áªÆ?îa‡ÌNàª?•—Ëí''?ƒw:Mïú?€þŸDh?¡¥Çêýl?C.ËF'?ï	1‹Ë‰?‹=Ë}f‡?g¦_áð{?a•§^*Y"?›äþš'¡h?Š`i/G3FGL J1917.1-3024@4¹£$\×À2x/øìˆÀ9MG8£µÀ;d¿1ٖà¿íž÷ì$Õ@¤[«Ltx@å6ÿñga¿çù@Éì¿âÎSEÞlÄ¿Þß4½eÀh¿ä$×3"=UNASNone?íá
êÃS¯?±;è8x`u?x±bÀ"?v¡CŽÕ¦7?®ë›'rÄÝ?°'ä߯þ?ïƒ5ìbä?';Ä3?gÄ¢L§Ò?lYeÏÔZy?‰A\TO…?^ŽÓ™)?í*ÉLօŸ? ì©lÿ$ö?œ×Ëþ?‰]øÉX8?®çá%2#?š‡CWa?î#\×ÂP?™Õþ5Á¯?Lþ©&'‡J?P¹-ûP?¯yύé"ì?™­аLs3FGL J1919.0+0452@D76z—À¡±–¡À9!çû&|lÀ:½;ÇVkG¿ÆUm*QQ@2ÁÇ`&@Å'ßÂó°¿á•·*ã¿îIîª(nD¿Éy_+Mz¿åIĸ3ìUNASNone?Ü4€!ð?Ð0FÆ~®?|@ŸKþq?'" n¿ð?á­ÆvW?Ð?1çú8?çü5Q?гZCk'Ú?ž&üM‰™?£v3`V?ÐxB¼Äû?Ï"£TÍ?ßIŠ+Ýä?¹ù®ÈÂjÑ?´Î¥+Í?¢V2z®?ۃ:+îÙ?¹ÐčÅÒ?ä äwe‹?Ã
sº}Q?\¸\ù6ó?auTéZåt?Ö¢X×ï¬?ìU«g3FGL J1921.6+1934@JÝdob@'T¡B‡À9,¶5±'µÀ:©-Ú-Þ?ß6ðôfÞ@
òA›«Â'@òÛ¿®×¿ã)¯–Á¿èÚZ~%Ë¿åw‹Dl@›¿ìÌx('2ìUNASNone?»Sp¢º?¸mäNÄ?ÑnVþg9\?ΐ`\+?ã媸?ϗÓLüÖ?à+úÞV0W?Ï3ZbÕ3"?»³wj/?º »—:cv?Øç]eŒ"Å?ÌðVÁez?Ò¯ù–'?µ@ó%Æ?Ìm"½^Ç?±Fp €<5?ß'çÄ
?¸²KZÍ?Ò$Åg·¸F?¾ÛØg?µ
¡f$­D?¢÷Í`Eæ?äKé_Ž5?Àb¡ïBtE3FGL J1922.2+2313@L'Õ'å!W@B™ØƒºÀ:CĆ­-ËÀ;nÏM°Œû?Ý[ò¤ÍªB@4˜³•™/?ùÿTžè¸ç?ácØl"&8¿ìl‰‰3Îl?åD\Ñ<H0¿ºhkÎUNASNone?îÓG÷6ö©?«—;j¦C8?2æÊ6í(T?4ÄäTi?¢¥²ø"»#?«Š¦PÍ?æ%%ºm?Մ9ß8dm?†Ë¯mºÑ?•1×híÆ?ÒÿX["H?Õq;)û£?íç°šµ?¢5UÇiÌ@?HjÅ¢Üî?€QhÄý¸?³æ¬Ñs? æ+sôô«?ï'h$^I?£CóÁŒ'?!±%Â,?:ÄhÛô^?Ÿy'JNtÁ?£× å63FGL J1923.2-7452@sÿ'}keªÀ</Ý÷vÅÀ9ŽŒŸ5À;ª­œ…Ý$?Ûs!ëb90@mdÆ~)&@¿¥`w9¿äh1à«Y"¿æå"Ód—¿ÚƒKÀY>¿â®xŒ6bEUNASNone?ï .<€i?'–ä
!©Â?MÏégY?R}r¨oHÍ?†µàÇï?'kÊ "j?ï'4•Z¾?˜#öŠ»è?uÂ䟴£m?{Ïpröò?•¨´,»K?"{˜ï-?î'Ô¦?1?"aú[¶Î?ˆÃ:¡g.B?xœ¼-š×? ±ï½BAd?è>%¥?í©BÌÅçö?ŸšL'''<?s¬è
}»?tbKTÙb?±{øä˜?žŠ"Åb–3FGL J1924.8-1034@;("ƒ‡ß]À(V*€JÀ9ÓôzùÀ;7›~v'¥?«x¥"éœ,@™Ã
+R@¾¦ ™@¿æ'H"¬:¿åÆ#aÃ¿Þ¾ø+}æ¿îÁç«lÍ*UNASNone?èô~³[Ù¶?ÂÃ<âߓ?·veLeÔå?´q,œ°?ÀrҌ]®¶?ºKDý$Œ}?ê'z×»?Ã^îÀ"þ?´\Á‡¯,?´Ç©Àõ@?ºê¨J˜?¸½–A—2?åÎeÉéÝW?³³•Üdçä?Ä&&~ÞV?ª•êhHy©?Ä­B±Ù¬P?©ç]åþoa?åV&?Åz?´œQ$Nâà?¦ýP;{æš?¡ÃBXøa?Òt	zxø9?³êHdÈ+[3FGL J1925.4+1605@IŠ3:}ª?zíݵõ'5À8	êâa‰ˆÀ:,îÉvÖ÷?™çÿûoÅ@µ…7âÅ]@À ý¿âî‹ÊŠ9¿é&¨¨L²-¿çM=«mh¿Ýü3¸ûDëUNASNone?VWB-á?†e3Îc?›Â6ËÖµu?§lÌ;˜9?îܖ8DA?©Í´k´çt?Õý´a¸?¢Mº Ή¢?¦"JIï?¬vß$SeW?îRÃdž*?²BnŠ±Â?¼–"Á?¥…ׇ·¥V?Ç>)[rÈ-?±_xÃL$?杣+K\¼?´ãd•.÷þ?ɜ^úJÄ?½6o.Ė?ŒëÉ:j$þ?1¦a(&?é%9VWĺ?¾òó á¤3FGL J1925.8-7826@s¾ó¶E¡ËÀ<@ýâïNÀ9¢îš|îhÀ;m溴œT¿´[jƬQ@
¯G·Ï @`aꁿê4,s,À¿äøã5U€¿á–"ö¶;¿ïÿÞ$8 UNASNone?ìomÊô"?»¶ÉÕ/?'õ|•J?•])K%?¸"OÔI6?¹vK¶q%i?ë–7cʎ?¸Ü߁?ó?ªÈ'îKGu?¨éˆ±BD"?µéûj…ç`?±`n±Â-?êN C"°6?¨œOJoÜÔ?³Ë¦D8]Ž?›}u3é.g?¹¿W¢² Ä?¡ÔÕõËëX?ç8r04?²À¸Ì< œ?§þULšuN? ÍGC-›?ÍûŠK¡Ù?±ÊÅì3FGL J1928.4+1838@JÓý`éNä?âz
w·Ç'À8‹iŽ9GÀ::
fðÏá?Ղë݉2™@
ÖLØ À@S%?ªá?âPîû¿èŸÛð¿è³ü"±E¿Ü3?_2âÎUNASNone?ªhÞ–?"¥ã¬U@¡?ÁÈ
‹*]Ý?Æ…¥¤
?뺳'ð?Æf*¡ÿïi?¡áŠµl^?²™Eµ
?¤´ë/]X?®–£¯M•5?향…ü³d?º9–Ë—Z?ÂëlóM¥?©¬¯(*[¯?ōþÏõ?°þÛ붧?åá¥Ù¸š?µRE&0Sà?Évj°ÉE?½Qâîì¿?˜9×µêâ?˜Šw]¼å?èà––%zX?¾"ÛœBe†3FGL J1931.1+1659@JBeÛ
Ø¿è…uŠÆ—ÿÀ8›Âª4À:DÏkã}é?õekÒa^@žûo! å@üN¿ÓÀ?ßðÉæ,^¿ãÌjoEĿ麃㾛¿ïÿA¡DUNASNone	?uŒÖ$êÏ?vŠ
÷ee?ån¡+?ÍÂ1Giù:?ÔÌGeEQT?͞e$2Í?sÓâ	±ž°?‰[)¬9ãg?Üׇ,AÚÑ?Ì8+Üî]<?ál"¥Ë¯[?Ìn^,ä?©šAgÔþ?–Èå¹Qá?Ü¿š
ÐK‹?µ#oÿ³WQ?àŽé±\ê?µŸ7e±<?¥+v¼?›òQþލ?ÜlsH;2?Â,s'Z?àwX*j?Â'5<Ø "3FGL J1934.2+6002@Vôå´$_[@27Mœk2À:Uî²ÑÀ;ö-±l¿Â†J~˯c@˜zãKz@nÿg(Ù¿ë³e"®£¿ÊlLJE^¿âð´ÁúG¿äKR6·)ÖUNASNone?ïÙ1h[PG?sQLÏõÐx?cTt«"'?jåö?cz"ù+'¥?eÃH¬¥Jõ?î¹®¢.B?¥TÞÌ¡?"ü¬@§Ãµ?˜)¸¶?þ¾?"ÍyúD?š'Ù'yOÊ?îàKô@Ú?Š›T
B+²?‹	[Þ.?}R
ŸÀ?–qï2ˆÖ?'ÃߦùyŒ?îBIÅa÷N?˜ÀÓü?•` PŒG?Š®2m"¼Y?¡+šg?'ƒSðÆ3FGL J1935.2-7924c@s¬Ç£˜ À<£IàâiÀ9z¹9r•À;J›'§å?ä1äèç#@€9'ù@|#ꬿÇI(]ANª¿íOŒ³é7M¿ãÒìa›."¿Þ$Tý¢UNASNone1?îžêI-¨?¨ù N
…?vïÁ¨?y†&%døä?£Nº	I?¨ÜdQw†?ï@ý›ÙÓ?¤å.±"¼Z?{/Œ¾ƒpØ?‰&ž@ÏÀ—?™ýãéu? ÕRï2ÁÁ?ëœÂZ?¥xë¨ çÆ?¥66
7ß?'Ïüq'?¸"½êY>?¡n
+È@ç?èrùÖÐB2?´8¤ã~'?ÛV=+1?§>ÃÍL?ÌbÊï[$'?³æ	z©±Z3FGL J1936.6-4215@vJ¡BoçÀ9Õõ'^éšÀ::7yéÑÀ;³¢/jP×?ðº<|]@ò¨ À€@w)¿ìêz¿à
TYôh¿Õ¬¿;>Åc¿ê¦;Ë`ˆ¿ïÿ…'yåtUNASNone?áÏCø/?ËÇÎÔ?±(?ÙÜÿΗ¸?Ì*µAêk?¤-ÛÂP^?¥·ï¢€ûÇ?Àp¡¼'?¼|ò}l^?åÊZÈé ®?Æj
BZÑ[?Èeó ;ì-?¾Ú^z1To?âñÞ´[h+?µ	ÿ8vÜ?Ññ…˜†b?²Q³pÛ?Â(¢#aR?§êœ…'	?Â{méÝ?®q]`®?è'ál{?·ue•ˆóŠ?·ºše°j?¦ê±»‡Í{3FGL J1943.8+2518@NœwškP±?殧]Q"ÈÀ8ÑøAÆÀ:œÁ>#Q¿Ï…·3@
›WœŸ˜@Ó0?ß|¿ß	-#,]Š¿èwu[»e¿æN¶¶#׺¿ä‹oVÇYUNASNone	?ž+ðo"Zú?¤¦]'ºˆã?œyt')ñ?¦_H~s'?î*ÔØs#Ù?²k'Nܵi?•:‹*Úd?©5¾äi? ,/Àò?¢¡ÎžÓ>-?îSk4Š§-?±Z«°ÿ?ÑëÜ¥{S?´?4ŠàÞ?¿Á&­H"?¤»ý'˜˜?ã"QìיD?¶Ãð›"M?Ýϳ–[Ö?ÀQxžrC?…ÌOoëË?€	è'QÞ*?àÀôöö'f?ÀZyœÛ3FGL J1944.0-0535@@óò^VÍlÀ,u\WìÀ9ðáù"»¼À;D"uuÍâ?К"»Dua@|Eëòè@ijàֆ¿æגMŸð÷¿ìð¯fEÀ¿æI8̶b¹?ÝڜÝàŠUNASNone?ï†T;2ƒ?"ÄîΏ?e'¨¨Ô«?k™ªþÃc­?‰!þ>»?" ¯,u?ﬨ@ì×?v ¥¯?\³O¸"©?r1ƄÑ??†28d?‰<«‡ô?º?îf€ÌÑ?–@Ç31)R?'KqMˆ¶?€¿Û$tÓ?¦Fù_Lnˆ?'m?znž§?ï'–'ÒoT?—W[%n~;?*Îã0'¶?CX³yw?š×ßy´ƒ?—P¼mV3FGL J1944.1+3919@R^ÞÁÁÖÐ@V:ADmîÀ9Ý|š…RÀ;€½I¢¿Ã‹
¯ëëv@
,"GÓ@yğ»¿àôõG6¬¿ám5Ù¼Ûy¿ãä$3¢*¿æn`I°'òUNASNone?ît'dæŽ`?¬.yP09?wJo.O>%?‰j!xR€?¥Í›ËÍ2/?ªAоÕ̎?í¯²¢‰¡$?±5‹]·o±?|TH¼Ýà?|ËDžã9?°½*ç')?°~
ãÿ8G?íÛü‰pé?œl¶Ž˜?"Ñν§vå?"Cÿxj?§×P
 	ó?–CI0­º?î@څ€$U?'—ÖèSï?pýX9!?f2òÖkÚ?©Ò·gò³'?óÄ,½":3FGL J1944.8+4300@S3¦µ(@"{¶NGÀ:Z©D1ˆ8À;¯¾ÌY	‡?ěáµ­E@
uËc–'t@!¿ím?ïæ"GÂP6¿Õ{è7È¿Öü}ù™Î¿æ̟m™
¨UNASNone?ïbŠ"N2?—·À_U]?h÷©³'Ó?nÉ+9¯í?º?Ébþ?–U­å´?ëäµ¢âUü?¿öÜn²«Ô?—÷5Qf8Ó?š dš†¥e?ºÜ…""Áò?¼÷¡–w"?î¢ä^Å?˜ª6$yæ?"bîâÄ}Ñ?ƒ†	'eR¨?¥ÄZH»ÔÑ?"3v±–L?ì–INo)ø?©'âóÂ?—BKùy?[0;¥?µ}"¥Qö?¦=¡ò… Û3FGL J1945.3+7329@Zd¾ß¤@@68üPHðÀ:4i¼\<AÀ;µò×s?ð9»þHoÛ@þ@ô'âÁ@XY …F%¿á1ÆT˿룠ÞÝE–¿âÔSÝUd¿ïÿ™`Â@5UNASNone?î7"Pf=Î?² VZñ"?…ƒ]eÃj&?Š¼9S?§%ó +H¢?°Æ8œsßÉ?áp÷´Š®?Ë(Ê`F?Øeáã?Ég™2ïVÃ?²èH¶[BV?±bÐﭛa?èÚS''9I?®
Sd(‰>?¾® '̃?¥D¿µG¡s?ºœµÊãi;?¢	Ë…?ÞHW»ÇÛ?¿´q,¬Aý?×0‡ˆI©P?Â8‰ûÈ?ÅBÍõ©?°¦ŠÛ"3FGL J1947.4-1121@<æÀ§¨À1'äy'¼À9À=h@[:À;coF߸b?ò¼¥¸5ç@
Ê8ƒW
@9T h«:¿áã¼üS¬¿æ[Ëû
¿ãàý·©ê¿ïÿÆòmESUNASNone?Ò]H°J:9?Æ4ÎØ KÆ?ËÓµEmó?Æeƒ~BÇ?߸ܬÿBO?É8á'÷c?ÔçvèÎê?Ægƒw?ÞGµ™®?ÆSl{T­?Ê'Ã/úq?¾AD£;½?᜾N5?³	'—™?ÐÖá¸f'C?¯ò%ߐ¦?ÇáÜ(9¤?©ôXE‡"I?Ó‡º_ÿ»?µ iw'¾?Ù¡IfRö;?¾©*ƒîr?ÓF.ßM
?µ݃hªV3FGL J1947.9-0743@@0,ÂÖ©ÅÀ0"ý*bªÀ9›A<á1ßÀ;WæáK	?ä]š@ÀgŽ¯…¿@= ˜ò¿ÅfÈ/¿éԇõ¾nÌ¿àiFî?Ó¿ïÿàí¸w"UNASNone?îóÒ?£NÁv^@G?"YýUâ¶a?ŠcQšrû©?—bÇJÂþ? óºI?ë¾zçŒb?»(§™.š?«æ%rž»:?©0þBç+
?´
L§T?³9}65Î?é缌ý?«ÛÇðl?º4}£¶5?¢æk§%y?¶'Ù¯áå?¢|*è&ø?å";®Ó€Ö?±|%"Í­?±˜P8·?¢Ÿ¡ôÙ%?ДâŽJГ?°2'Ðظ˜3FGL J1948.1-7059@tE¤Ý/ À>#óYÿO×À:8	=–c"À; ±Po"¿ùë›oÉ@›-—
H@¤è¿òsпçÞтFÊG¿èÒ=؆¿áɆµwÓ¿å"DkÐï­UNASNone?ïÁñMÛ
T?/1¼°h?@…¡AÇf?DÇS/ŽÑJ?|ö¤ê@ia?Lє"?ï•!¹8:ï?';[ÑVºÄ?a‡´ùֈ_?t˄£Û²Å?†U¤s{¢B?¦
PgŸ!?íèŒò öN?—S_ä7[?Ù__9·Ã?{яœÇ13?©
&S¿R?"‡5Ç(á?îàe'?˜v³¿Ó+?1Ö.q	œ¬?6MX?¦
…œÅËB?˜f´<‹V3FGL J1949.5-1454@9¶¹ä'¼0À3v…3±tÀ9´ÒŠ{ïeÀ;n"WBÜô?óZ¥óš@s¯H'zÄ@Ž@À9–z?ç=Û­»:¿åJÁI-gå¿ægò(b0¿ïÿωþœUNASNone?æÐ×Ävº?ɓÆð›?ÎÀ‰¼»?ǧšÛžÊ ?±ÀeÈfF?²Oì¸9€_?Ýq|ð
—?Í©ùl{Ù¶?ØÜ"«À?Ê]ÀAŠÅd?Å©dÀÈi²?¼úovË!+?Ü¿BzÖ}q?·¹vÑdV?ÚpÿÑo¶?¶¦c_yn?ÁŸ{h,%°?¥ec²ù?ÓÔašY?·1º"ž4?Þ¬@´œj?¾5oP''?ͤþ»b*?·2ÄÅ
õ'3FGL J1949.6+2355@NXG¡A)¿ñ×Ê÷àvÎÀ9#ª¥æ¯À:€Ú†?à2»œ"àÖ@7í&ßgÚ@Z¶ 8Ò¿Ü·N´ ·
¿Ö³'|¼6¿ì"žZ@	Ó¿ß21k

UNASNone?®'‰ßDž›?³dCz\ã?Õp`œ^]?Б¡
4?ã_§T½†ç?ÐÝWCœÿ?·íÛm}l?Ïdü?Èd'Þa.?Ç"‹ÖÄ¢?æé#ÚǤÎ?Ì(õ&¶N›?ÒuãV¬7?³]«C‰Y?Ƹüùb¸?­ó'ר?áÏdKÇ?¶S›1™hç?ÌõŠfBÚy?½ã3E@ց?ÄCF5'?¿ýØ}Ž?㱺âþ?Ãí!ÉF'3FGL J1949.7-8109@s‹ohÜÀ=ãæÄŗÀ9ÁC
›ÉöÀ;m±|å-í?ä¢X —>@VŠ16"@šwàŒGL¿Î"tŸA×Ŀ飨Dhuñ¿Ø©Ý ¿ê®iÆ~eUNASNone?ï¨×ª˜T?ˆ í¨ ²?k/ó/?xÇð©Æ"?}ü¶10R?'£ÿ£g?ï*0éü½?–îÀ±fj?uÀ›L·t?vê0(pÑ?•I»ígbR?"ͽ¯©•?í$…ÔΆ?£)–dˆå?¥4qû'ÖU?—–<™ ?¨ƒ0·¡M?˜2D¢,_?ëc'Ϊ?¦ÓÃþ`?'¯Éë´ '?~Ř	È2à?ÀØÑÔ¥ƒU?¥Ýº«}ÿv3FGL J1950.2+1215@IS6Þ¹^[ÀxK èBtÀ8Ù°i¿·;À;øìˆ3?õ…*ôö6©@Q¨ò'$\@à`}n¿ã
l"Y¿ç¨6©EšO¿í‰Îtäûº¿ïþfå^¶fUNASNone?Ùqò!Jc"?ȧ"Ï 
í?Õ²@ïA7?ÉæS"ÅÃï?ÐÜ	Æ[5?Ç2;V4? í¡+ÌÆf?©…¼jÿ?â¥äބË?Ȧ¦ÓbÎ?ÙÝÉ] ?È'Ý?Ùf©A9'£?³Ÿ^>Վs?Öy$z)?³;ÝW|?Ð CšLg4?°†ºÃf¬?¶2ù.h}w?¡ù­t`-B?æäÂ>fzì?»Ý*‰-ü?ÉSzo1՚?µ³Ä8i¹ï3FGL J1951.3+6909@Y]uÍ·@4#ãŸw),À9÷Š1FÉéÀ;À´4O'å?Ôîhæ¦ñ@Òbœ­JQ@•ÀoF_¿éí$
Ú¿ëÒÑøß¿åْ 1+z¿Ý.ÚáÆUNASNone?ïÐôåœ]Ü?{"åa©§?MðØ/ÔBZ?S\5f÷Ð
?sÇr+։ ?yi?J'5?ï{hcãY?•j™þ'2h?{ۍ§ÎL?"ÙWàÿêŠ?ƒ8 3Q›?Œ¡xpÁ¨?î¸4eX´?'
jme?†k´ˆÓæ?wµ(p¿ó?Ãëú©Ÿ…?‹Õø)µ?în[Ž(?œÇJÙܸ?|VW52'&?~@"ãÍ­?¥|1g-:?› 0öÏ3FGL J1951.8-1102@=°É2
™FÀ2[Õº²À:Á!ßyÀ;eºßd?èr˜7]©@Ûï«ÉòÓ@֓À;ÄÒ?ï_»eàô;¿Üѳ¼©¿äÆ«¦j%¿Ûy%è"JóUNASNone?ïtŸx("?'µ]lÈiA?z_´èñ°¾?ƒCš,ê"?…¨G~§f?†£wÅÆ©–?øõî?®óJGn
Ÿ?Šyöa¶àc?˜Bã#Ç?ž¯%°ò"?§L&ÎÝ×?íGÞc$]?ž›þA÷?¢Tá'À4?'äY?©-8:ÿV?""5w²{?åøYlŠÆ¦?º‡ÍµØ²?²™v®µoH?°
ü6óÉL?ÎÑÞöz-Å?··8æ¨îò3FGL J1953.3+3847@RzAc
'@~¡ÆÀ9T†È½¯À;
»3GU)?êU7°×‰û@
ë×j@zoÜÝ¿ÜòD…ëçÅ¿çÜ%ìèdó¿èz0¶èE4¿ïÿ™àóUNASNone?Þ3~ŠŒ¦?Éä®+Z?Ä$¥9¦Ä?ÀLÃNÎ=þ?׺.ÙR?Ê"Ûˆ\H?Ã|ƒØ«×á?À¿íz•?×Ö†¬|?ÇÞwÜP½"?Þk©#g"?Ên/qg?áQì0PÜ?µ•oö¹§?È6*–ã1W?ªt‡£*È?ÑA'-Ŝ?²ó˜GËá?Å"ó²*¸ƒ?¨fLüép°?Þ±*+"/?¹—tŠ°ì	?Ö½[ûڏ?µt3‡ìiy3FGL J1953.4+7653@[LлnÖw@6ö¦ڜ™À:;[dRÀ;Èp0ꃗ¿Ð1¬¦ÍÅ×@¸1Hwh@ØÀ€
V¿å>ú߄µ\¿èUDÔxñ¿åCŸjþ&¿ÝÝ=ÄUNASNone?ïÉrêÔ1V?¡¾Ò:ú?Z†ªÅyú?] æ9[xû?t¤ßòuö?|áV]ÄԄ?ï¶m;35È?'dìà´?lË<…S—?oi±Ÿ	?vcÄ#»Pf?{ìFŽá?ï0ɨ?Šʾ¤œ?'áDÈvÆ?vº€Ùv a?"5É\¦?ƒ}䯹yÖ?ïb,ê4'?…"õç`™ø?N'#$˜	?O­Sü¦¶ø?'Ê©IÈI3?…@'Aa3FGL J1955.7-7019@tQ!–R½À>ÓKµáÀ:p‹¨?NÊÀ;̽M#Ÿ?Æì,­Nœ@
+Š•š±@
@/p¿ãã…³¼8¿Ød™ó‡¿â1|ÇX¿á£LúôAJUNASNone?ïh~›Od·?"š!@öI?JF5"ÐfA?eGŒø­ž?'úìüåç?"A¸¸?ïIǏþ-?–æG(þ?p£Ô	¬?t?xR#s?'¶'•*–?"€>_¦8?î(Ò×®¹¾?•LØ®@jð?'/€žòâ*?JGŸÐªß?¤[5šòô?ÑhÇh…Ÿ?'Ï?•óŒNµ'#?~¦»Ü»ü;?xÙÚîmt?ªŽýv‹?"€l]'B3FGL J1957.9-0712@@ÿùÆ*\À2Ò^Ý)À9ÊØ>À;rȖg"¿Ð¼[\ê^%@
£prƒÖ@Åz¤6¿ã
e'ª6ö¿éÓb¾™¶Ó¿á"3©®BQ¿è‹Ãÿ/UNASNone?æKLã`T°?Ç÷å˜æ'?‰ÄÁ…®¢?‹fŒÒJ
?қ@0»)*?Ç®é3@©`?î°æ_÷F?©mUxN?†Y2£UM?0Z¹6S?ž¶šöML?¤#ʧK?ìb…9ò?§tçÓx,"? QUîF?‹Òþ³áŸ?·¶²]ß
t?£NëÞ¡rç?êÂÍ|Qrû?©&6‹[?Œ?{ëè~Öâ?sp8é?ÄjÊÃ}?¨à9hÑ93FGL J1958.1+2436@O#´·,ÀQ½í@À9Õµ•x¢©À;[L
ÀÛ¡šÀ`@Ù2¹e¼È?úÜjŸ01v?æM"xºžC¿àƔR̚g¿³4ÊþҔž¿ÛPý~"xUNASNone?ï8µâ'?£Ïu'ÂTõ?MkISdóu?NŽ Õ)Â?—ýõ"è†??£³ô¢Q?ç:¬Q'?Յ´#øJ?"¤|l\? §6»;'?Ðå'ñô'ç?Õ&	o«'j?ìÇc-œ=é?¥½Ãð*?"VK' ¤Í?"¶ETèõ?´ïSÉUç}?£Èlx€?ïø	‹é?û¶ÄE/P>µúŠkä‹`>Ëã3‹õ?‹ÁMÈê¦`?ûgHØݗ3FGL J1958.1-0243@CЀ¶sÅÀ0>h›À9‹•¢"À;Vé<o?ÇÂyë1@
O^b@ìi_À¿à—%oŒ·¿êðò	áð¿è9/B[M¿ïÿ®7¥!§UNASNone?íºÚi?±fé
Rú?ŒÏïŒC¦
?Ÿ¤‹œ^fˆ?­*ãOOê?­I
Ȅs?é²Ï–¸P^?ònOã&?¶ÍÞ<}"?³äÖ8±ä°?»›¥<ÿv?ºË'ó•®?鼆:°œ?©Å¾7·"?¹í¦¿? N\A{ô'?½ù.(o\?¡ü×E¤~3?áÓ_nT¡¶?µxÌÕ>4?À÷å,P?¯T}賖]?ÓÝN‡?µ æ,#€X3FGL J1958.2-1413@;LŽÞT´À5§ÞÖºŒÀ9Õ¤9/ÌvÀ;t_˜?õ#¡Å¸@Ä
Ò¦€ˆ@Q%¿'6|¿ÀÈk%^¿ê!ÁduÍ¿íi=®ŒDò¿¨ÃG.ÇUNASNone?×µ<u°?ÍJËrâØ?ß~ýÁÜ	?Ðå	ԗC?Á—‹a]èa?ÁnUޑÜÃ?ì͂ÎV€?Ä°&ó–?¤Ñõ
&2š?¶‰úZf.?®UÞäej?¸ÐÈc=D?äA‡*ì°Ø?±Ì{Ö-½6?Ê.Ïè¡^
?­ð£»:ć?ÄËk«Þ'?§`-D59?â½e%`4?ȅÂá™ç?ÃÞåþ4KŽ?ÉS˜¡o¨¶?Ò6›Ï?ÄNJe ž3FGL J1958.6+3844@R™é9êÝY@hg~"Z•À9XÓÍ$áÀ:ﺽ֏Ä?ÚlƒÁH¾@ÉQàd)@PŸGƒ¿é×*'EÑ,¿èZAâÎkÞ¿åþ	WŽÿ"¿ì+€áUNASNone?îCÀuá~?¯£Jx?w¹ÜÆ®?}á
žª¹N?¨Ì½	7å?­NÊlUZ?êÁznèj?À×c'P5|?ÉßJÚ?'Ye<?±?Ã
©xO²?¿ÅÛÇôèô?è#¢$–â?µGù[hì{?°$zܘ?¼þ^š¸?Çatå¶.?²'x¿Øþ?è˜
®F?³.=0A:?"<S^Íçy?‡<ƒíBW?Ë8?n-ü?²JqŵH3FGL J2004.4+3338@Qªõs}¦?ò÷; ¿þˆÀ7Þ@c^JÀ:›ò¼K?óp"£¶S@WÉy[5±@^Ø_ýì¿àáÐûø¿æ]ª8*òP¿äË4àÝP¿åiÀBеUNASNone?¯{ÄE§W»?¬×Š.9A?ÊúςÅv\?ÆNO_ôMý?çIÚô,î?ÈjNJ}Ó6?¯òWìlÐ?¹ãŽ+F_?Ê,ɛ¯˜?Ã¥u>…ãb?ç">s•S/?Æjéó!UÓ?Ís¯Ê÷`?³[º^€z?ÆÁéýH‹–?ªbßc-3'?âò™ð'?¶Q—î?*¹?Åø¹!2œ?©šSäC˜p?ÌFÚzrj¼?µ-h.·?ã¬3ª?´ªh꽩93FGL J2005.7-8241@smÝ/Ÿ¾À=:úÖËSPÀ9ë:жfYÀ;‰$Ų&?Ï­¥EýÄ@ُöÏc@p0`E)¿ç"A¢¿é¶ÔÕ|@:¿â»|y(¿ïÿ­½Æ}0UNASNone?ïûióúÏ?FbîzÆ[?'|²f—^?^ü¨‹?@IÀ™Çó™?E¥Äùє?ï	6¾*v?8Ç#õr[?zGP‰)=o?~+ØiH.?˜GTuê?™gÛ¯eº"?ïÓ¸¬–?‡'ã-á¿F?‹ôaÉSÌ?y]4–#"´?'˜ëXÃ`?²M£U´y?읰BËñ¤?¦¹ÔÓä?‡]f.θ.?€öû5kp"?¸&Ñ#ƛÞ?¥9o
b3FGL J2006.5-0939@@Q'>EÀ5‹&9O­À:˜._ŽÜÀ;¥1}PŽ?ï™ÿ¤ª2³@õæÌ}G@~Ûÿo·H¿ÜBÈÍ
åF¿éC¥×?—p¿ïþOÃ%ã?ïͦ¦óIcUNASNone?îOñ—°?³$:aµþ?ž"f¦Õ(?¨¨¨ó¼±[?—‹ÄyF4ß?§·$Âk¹'?îÜô'Ñq?·­÷"¬1©?…X–¥%?£Q1oûaØ?™µaZPö?°'2"m˜?ê…'%âñ?©&S)Q7?²Vœùå3ô?žYˆ'#¤?¹€)×
d†?¡cºtã	ö?îŠPnrÝ?²ˆ_û?'Šôú??¡otÕ"1u?©tºtñÜ?°èÈøO<3FGL J2006.6+0150@E¸²•éá±À/aǛ4¤À:3ùJYQÀ;›zé¯?ðÝ ,e@:%Ïrn‡?ýô€kJQ¿ãÉÁb"ü?ïÍØWiJ¿á`pX
a¿çµ>LòUNASNone?êdœý‰?Ž¦
Y¨½?¤ñë)ÜÕ?§äwËÄÝÚ?¾3nÁ'¤?à®úÞIî?«$ÖP¯}?Æ+Š=âù?å߈¾.?ÉÝ(çéÔB?ÅÖ¸1ª˜?ÀS±úΘq?è©ã­¤?µo:*é4?¸"þÅ«Z?¤G+¡q
?ÁqèâLd?°mÞëë?ÅúqQÁ?»HX3=Ë?éc;é0Bõ?¿°ë¤3/?¡â}´Ì…?¢Øðñ³.3FGL J2009.2-1458@;³íÇïzÀ7Ôé8yÄÀ9¢eYöì[À;d¸€åm®?ñK×+Ë_å@i›ô<ÓE@' ¦Ô¿å|!SŒÄõ¿ë¹©#Ð>Ç¿éŠp|h¿î¨#§Ù›UNASNone?ÜFAEä݂?Êɓ:±n\?Õ ®tj?Ì)x~‰Ø?Í3>Mpß?Æ=['×Q&?а¹CXË\?NJáU?à"Ÿôhæ…?ÊM}°©?ÌP
§ªÏ1?À*‰à!¤?ä
aáaN^?²
zfJÅE?Ë7GŒ¥÷¦?­Uß ?ğ0íÔÎÞ?¦³!b3—?ÃàóKZ†?¯¸÷͙ý?á|ûªlq?Á»ØöJR'?ӏ›yÛ?»öiBpÖ3FGL J2010.0-2120@5Fw_²íþÀ:f	EùßUÀ:.P‹2ΉÀ;¤#ìnS?ñŠ¢`<«­@
[ûÈ7ç£@l€xá=?ïü[J ¿¹i8þ6AÕ¿àÊÂè-·"¿ì¿.Äí
UNASNone?ÓªZgP—^?È^Œ­åê?â7íx[÷9?ÌöÁbv9Ô?¿—*ŸÝè¹?¼D':ù±?Ó9{:ö"?É©:ùŠ¨g?àV5ýÎu?Ë.0>'ú¦?ȆµP>‡?¿(éT´†?ØüÖ|P±º?¸V¦»øåë?ÛÐ
wü?¸Ûr׫,?Æf.òn¤{?±'郇?ÑͬÁdPü?½6ÆE`Úà?âÅÖ¦1ø?ÂTºØóèò?ÁMKäږ)?²/{ÞÇ¥‹3FGL J2011.1+4203@SŸ …±…I@_î} ½À9?Ú{9À:ÈTà,%"?õa
1@ë@
²ká$ž@I« §U¿æŽXõÜÝÞ¿ê÷å#¿æøá–ïi¿ÝÃëfjUNASNone?Ó
Qî³Îô?Éùàoâ0V?Ã}ÎõÎè±?Áku#ßD?á™ãK2^Y?Οç<cFr?ç/;ƒy<-?Íëð¤ˆV¤?ª÷	dæ?³º»KOj?̅O˜áŽÅ?ÉPP€t?݊kÎqÕ?µÚ®œ¥?Dž5X¢?«¼\'éÀ­?Ö³)ó~ª?µköÑý¯?ÕZ#c»|á?Ž¶J͔?ÀµŸ×e?Á`ð^‹O?á%¦æ,h+?ÃÈ)ôÓ3FGL J2014.5+5246@Uøígwž@#Ìó˜éprÀ:3o­7PÀ;k¹Ù&w?íRŒ#†º;@#¶XzÀ@bÿèƒ¿éõ'–âd¿ïÿžæWê?ïúu7B?¿Üº ÆUNASNone?ï€~¡+ó'?ª¬PO_/?K©ª)6Jô?Wƌh©F,?Ž%½o¶ñ?ª†ÉA‹¶?ìóÆÅ"™?Å%³q ÕQ? À…§Îy?Ãñ%š‡?¶=±Æ6::?Ä àbe?ìòÂïW#?£y+JùØ?˜@}lÊ3?Œ!9‡?×?²Yë™*^? º9s?@±?îpú+Ú$‹?´‰T¬pŸ??ž""è[T?hhК~?¨± 3æš?´ƒ2B™j3FGL J2015.3-1431@<ÎdÜY2À9oç¨mÀ:­{έxÀ;µ}Ëùï?ÊÈ­Ì_N@úٝj´?üSQ@g<?Æ]E¶©•?Èk"…þŠ¿Þ{V¦-¿ 2
W!<UNASNone?ï¯
S'`?"¤«'Êh?Wp¾jÀq?aCS'o`<?N"NCÙ¨?' Î¸3?ïâñ§Óø?Š<³"Ô&z?`û}5yš?fZF>°:´?"fĶ½£€?‡Rj¦Â@?î‰Hn;½L?Ž 'ÿ¢F?¼N!úª?úâOÚ|2?ž¤Èç?†TN	¼Y?îÞò6Ó?–‰ÝV?¹?p·Œ0Ý?xr¿9ñòÚ?ŸóøV3¾=?•L2Yì&Ó3FGL J2018.6+4213@SÙÆ*\}@>"ՔÀ8wöº «À:€
è j?ñŽÑä›@¨RÙÛ_@&«ÿÍ«¿Í¡Bt2œ¿ëAlKO+.¿ÜáÑÁŠú¿ì
2ŽÈìUNASNone?"½žñ¾ö?‹¾ì±?J?Æg'€$È=?Çbi¥º?ê$ä/Õu?Ç«±=
¾]?¶qXˆ¥hÍ?»º*]ÚWB?Ù#­/Ô·?È/gõë$Õ?à P˜Sh‹?Éã"Îâ$‹?ÀôÏr?¨ÞíSpMŽ?ӈÉ
Ž?´QuÀØ?áþgœ¶/T?µÌÌkc9
?²ù"˜jۉ?¤Ø.­Fä?ÇK¼I§+?·åHԘ$?çÍÞZ±zÄ?¼ª˜äé3FGL J2022.2-7220@t%VÿÁßÀ@LOô4ãÀ:¨t"ÅÀ<ÖÝÇÆÔ?ñ®hk#d‰@
>§3á?ÿ0Ñ@úÇ?䶄OÊ1?Á¿œS™k]?Ö(f")_l¿ìÞß}Ú UNASNone?Ù2p!Ý
‹?ÏôRTü?àLa©?ϕuœ.Î?¸Ò4p†€ü?¹bƒhñ´à?àŽ9Àìö?Ô4'+½ä?Óçä›P'?ѺÄOÃ*?Å÷R'[þ?ÀÞèØ$´?Û¯ä8¶å?·íÑ°Uÿ?Ú^!þ5ÊÝ?·!W¼Ë%?Ããó'& 5?­óÓÞé8?ê#Ê>ð‰‹?ÄOódÉÂÂ?»¢"¾[ÜQ?ÂòMê2m?³?‹J×Y?²ëÕKÊÁ3FGL J2024.6+0309@Gzš€If{À3%oü^À9ûUê`oÀ;€.ÓR"?ëhSÃ÷f(@"ŠÝ"T?þŸ`A^D?âa6FÒ¿Ó}Ìyjп×ÛÞéëý¦¿ì¦˜	UNASNone?éó=›ýƒ?Â<àúì?Ťl¬±)ã?Á™>XÜß?"tç9÷w?—"S"'›Ú?ꐘɯf?Á#…˼ô0?µÎ[Ñþ…?·ÁøOª±h?µ¬ã°©†L?²òP›÷Å?ä"Räï|.?´D¶I_ûö?ÏP€|(>X?±@ÆÚd?¼Ägà3¡â?¨Gl¯ã±?æȄQ²²M?¶÷XÔý=X?»ÂVƧ?¯!²»éÂ?ÆüÃUá¨K?±¾õdË3FGL J2024.8-2331@4=Ž§ÎÃÀ>\ÜY1ÊÀ:'ý«'é¢À;̝{¦iŒ?é;H›¹|@
ßþWß:?ÿ2¼À»Ÿ?ïø̵O؅?ÚQY1¨!¿ÑçD6"¿ëŒÇÓá
"UNASNone?î$"¢?­±DÕÁô?£©76àT?§!Ã&v‡?"-q¨ùë:?š˜O&ÎÃ6?â
›µ?ÎÉáO Eó?Ñst"Jà>?ÊqgÔÀyµ?Ääüe/Ъ?½C¬^š?é'¬!Bâ?°#éÓ?Á¯™EFH?©o¡>œ{?³eálk\`?¡ˆNl"Ï?ãÇ{†¸)?Ť3fÌ'?Ó#"RÍñw?ÅÀk-*ؾ?µ7š€Bxâ?®fãý}R?3FGL J2025.1-2858@,Y'fw-^À@"Ý—ö+À:TŠBäÀ;°®Xm_?ÒÓ¥ˆT½@ñ8Hñ¶@}ûŸž¿è…¶ˆ×n¿äÍD¢úÊ¿Ü?Géxª¿ÕvØiþ»UNASNone?ïÝl‡ÇLæ?p'3ž(ü‰?,bu$Ÿ6?/¼(CÑNõ?pf¨s8Ÿª?o‹³Ü0üÃ?ïI³ÛŠÈö?›´"«ù*?o!å¼±+?Z´\ï?'åbïK'?–¾¿O÷ß?î¨À}|'A?Ž(¶Ä†Ô?‡8cÎö?s¡o}NF?ŸK¾ÈàPu?ˆæ‡>
Š?í‰K 0>É? cCkÝ*,?n¢<kâ¤Ù?w/¿‡È?²À•ô? òóLYÀ3FGL J2026.3+1430@L¡WÞ
fñÀ*àÔº××ÃÀ9΃&À;˜(ßó?çN	÷^@ËoT¡˜@E¨@P}¿Ê/àýJ1ì¿än¸oüõ¿×û'hZK¿íi$;!GUNASNone?ë…I/bФ?º±»/œ3ù?µÙÍs¬?²a"}R~y?­¥¹o´f?¯Jõ€L÷¦?êRʴǂe?À9ï–?²Ò?²Qcêw›²?­Æf–•Uº?»FoLQ'?·Ü
H–?ç㊥º[4?²Š/¢ÇR'?ÄrøÐEu?¬_` ëp?·ý¹1¡ëu?¤ñ¦"¯s?énÎë>=?®zo'´˜V?«æ
7ÈUž? ÓÊz¹^&?ÃKAöR?ª
€¡}	<3FGL J2026.4+4709@U-Œ*EN@ÓáF×UÀ9rÀdß}©À:ùbLLà¿å|°R
 @ù|ÙŒ@|Þ 3玿â,»ç‹Y¿åƒ‹Ç·}¿í87V¯¿ '÷Ö:ߥUNASNone?çŠÛkr´¦?ÈÛöjd6?¥µ=¤r8à?¦d³‹XÏi?ÌgBéŸ1?Ç¡àÓ¼œ?îSÐZÛ ?°
BPŠ?p(IcT†D?|¸TŸ
6?¨½ñ+wµ7?®yÛÐrûÆ?çîÝ%]}m?´£'™»Þ•?±M¾—èbÌ?¡×)«ú!ä?ǝ¬•Øê?±8³ùl¯?í×òp'£Ù?¦CÊP,2{?E}â6R?Tæp­{?±S€&ÂÇ?¦7öÝ×´+3FGL J2028.5+4040c@SËà"&þ?ò[·¶»À8ÑhÉíõ<À:O¶1ÔÌ?ôù`[µ]o@š
Wǽ@р:ÍÜ¿ÒÅÈ*j{Ž¿á†qŌ‰¿ë_=ú"¿ä~÷õ·UNASNone4?€¶³­;|'?‡!Û&ñ?΋Ž9}ˆð?˽Ÿô*¼Ï?èA¢ë¯Ó?Ì
'Xöý?Ê8>§TË?Ë¡[°ñ‰?¾ṟ01?¼æoàÏÅñ?壗ä"Õ‡?Í4墑Ö?À¼C6C ?§œ+¬ƒÝ€?É×ُëJç?®æ4=öJ†?åZøÎte??³ˆÊÑfmä?Ã%BHФ°?·ˆYE?džøÙÊÓ§?¾È'¦ðIZ?åTñ7Y!ê?ÁJ¦M‰Wz3FGL J2028.7+1012@JëÍþûôÀ0Cý?[_¢À:ˆabñgÀ;vJt˜XQÀÎރ®uÊ@ËFºÏt@ ¨?ϣ¿èº"Ÿ"€Å¿èÀží°6¿åâ'ó~¬¿Û†u¾%ȚUNASNone?ïÅ6,ØI?ØühZ^´?a]‹'ì€I?m;µµy?t¶$3›o?}BpǺÇ[?ïŒÎÃÀb?š}ô{-ƒþ?gé(6ö{{?W Ž¬[?†Ò/ARHµ?"÷N?íœí‹ëz?˜vT'""?–JV2Ÿ¬?"²&°
áa?«!L'ø?"O²<=h?îo:WÀ^?¢f·"¬%?†­
?*Ó¨Öpÿê?¨ü—;ôs™?¢c¤ÑOÙ3FGL J2029.5-4232@ve†á›ëÀA¾^9q;À9Ö-Š|Æ$À;±+hc–¨?îsÛïÕe@
|+Þ«¢@öã•Ò¿åæɕµ´W¿äd"p 4º¿ídÓÈÙ<¿ïþ†ìwUNASNone?ã]ÅEÍH?̯…ÿˆ%"?ǽf[°'%?ÃÊIh@?Ê˄Ü£Á?Æõ5úsÝ?Ö7K{`¨?Çha™:Þ?؜{®¸>ì?Éz~ÔÅ-r?ÑIMÌ`l?Áœ"¢Í7A?æ³l4^I?³gҗh^m?ñ¨Æ>ª?ªÂ¤QØ¡Ÿ?Á€¦hh?§"•w§?Ð=¨}õ?¶ÈY±…?ãXüÌ%t?¿A=É»Ž?Ã?KŸ€?±½p_},3FGL J2030.5-1439@>Mã†Lµ»À<nš€If{À:¨ÂD³Ž7À;ÕäbÈ¿×Ûâ"Då@
h³'Š2ž?ý×>Ý
ˆ¿´SÅ)Åj¿Íºòºr,B¿àÒ­›rüf¿ØZg!ËËUNASNone?ïÁ"xÛR¨?}8O|Õj?P=)¹ µ?QRäVµ9?{_y$£…?|?RŠ°n?ï®(ÿȊ–?'ßÖ8G®6?X·VL¾wr?]~¦==?^ÕDE‹Í?$*[)<?îšÝ¤;?Ž?2Mš?'¯&?PV?œ7½ÛÐ?œOFdû"™?"b¼Ê0þ?ï]¦Æš50?"'T¢Ø+?Gœ!É0ªî?IO¾†ÆßJ?"ŽFoԟ?"=ÜË®%ä3FGL J2033.3+4348c@TœŒ" Ú@Ü@Þ¡À9Ý©"â À:aþ£®$?çbŽÀwª@
c¤&œ@ð»`å5?ï÷Ž›Ðù¿ë¬Î
 ©¿áÀø´îc¿ãmϟ™UNASNone8?º× å~8P?Ás¾HC5œ?å™ø ?˜Osz¼»?ì(ìLèVv?‡JgNã?Ù|	Ž?Õ4k=X¹?¬/O•ž»?´"†x@M?áßÍ?ÔXÝý?К)†Q™ü?´¬±sÝ&â?·]É} å?¢fʵgõ1?äÇ2
6^å?·+u[ô9?ËS麲4?¾Y¬
IÓ±?œ8mÄ?™÷6…Ld&?èKÍå_?¿Ñ^zĵ^3FGL J2034.6-4202@vq9C¬ÅÀB0øµˆãiÀ:~L69xÀ;©Ù¿#–Þ?æ!;xjä"@
éåµüÑ¢?ÿ+žÔA
?íåÐ6c¿B¿ç&çEsý?¦®o§sE¿é"ªß½sUNASNone?î?›†Éá[?±сŒ¦?j«L×\É$?nc8﷋?ª['Åìº?°¾Ùe?l?íÂã¹w?°‡ÐX
"?"Ã?›§ì÷Rk²?ª×>%®l?§ÉûÆò?쭒ç>Ų?§
΂iž'?¥ÞÖô³Ô[?™jEÉ!)`?¯Gú—_Љ?ž±Ùnä|?é瘢ÏÔ½?¸êéœ|–?2͝ï
?–¸â<¤@Ï?Æ[CÁï*?¸*â
uÐP3FGL J2035.6+3146@R5ËÿGs\À(IёXÀ9‡â3f^ÚÀ;Šyk%é?êTÕ£@…lP‹2Ï@fs€€C¿ë&FÌ'5¿ç¿¯æÀœp¿Ö50•ì]X¿æÓq†wuOUNASNone?íáÁí¿?±ÒMÃv¼?yù3é!+~?€+CéC
O?®¤º±é?±ŠOå)L?ç†ënI?ÌRÀ´†à?¡àyâ¾?¤Éê°e˜?Í¢WÚ):,?ÉÑÍ;q—?êÐW!Áµ?¬!#?'V?¥mÌì*×?–^¶£×
"?¾÷à{Üí?§$ƛwÊ·?è§grč?¸ Œ‹Ú.?yå›å¾îô?wÚD|².¢?̔‰ƒöX?¸u++h–3FGL J2035.8+4902@U­'#'@#M~8DÀ9Î.\3Ý}À;¨—š¼¿ê¢ä4â$@T(1ÍWŒ@Ãf?úìƿ䍙/*SÕ¿Î4Ÿ䦑¿æ¤
™¬Ë¿àˆàéiUNASNone?ìßFL]‹?¸KAPæ?']­'bF?"Ü+3¬W?¶ºþ,Ç[?·Tb)±Û?î$y¥?°ã¥12k?rŽÛ\?|ò‰Õ̌?¬+õÊC˜?°-ÿº2.ò?ëþé#}Y?¨½8ܒŸ-?¢È@Þ?'½˜|˜6?¶üRÙF–É?¤%'d2ì?íƺ
ŒÐü?¢nðâß $?XÁôº^Ì/?Zçžöd²H?±g'دüé?¢K—Tù'Ø3FGL J2036.8+4234c@ThÕ¥¹c?ïèV`^åiÀ8§1"ÉÿÀ:3\m¿ <?õ"åm,©+@
êÇ+£ù@"€U$ö¿Åˆk><{±¿é={Êaô£¿æ'˦þ'¿ç
Yûsÿ+UNASNone9?`î¬kÊÈ?aM#GH£?§Ðՙ•bú?±"~ø!Gâ?îrï·º>?±d߂›óð?¸È¤×ÃÞ+?Ãù¼CµÎa?ÁÚ®À
‹?À:­ù|[‰?èp?µáu?ɚy«Æ*–?ºT'Š_E?¢þyq5?Ä÷õßÜì?«˜>¨9àæ?çw¨?Ö¼Ü?± ÞjA¼?¸ O©Þ´?°á›ÑQT?¾‰ûóW}?´H5Ñ©?é,öŒY9?»½MÞÇ3FGL J2037.4+4132c@T7™E¶Ãv?ÒÙUÜ«g!À8˜-¹éÀ:2ÿâ£Î§?ê	ÑÇÞQ@
®¸–^ü@lÁÅm2?Âí'f²wÈ¿èôöЖ¿äM{‡F ¿äoñÆg"UNASNone ?b`Aº¥¸†?iæ"&m?úD"'z?‹ …*ÌVú?略«ø¼`?Ž2ÔûÐÝ?†'(»
¥¤?šÕ/tË®?¨;¹qō?©~ÁÖÈiž?î!ÿÄ¹?¯ü;V¹kl?¿ÌÏlá?¥)³¥{™S?¹r`
(þ?¢1†
è?èænúÁ?­øg¥Ç?Âa³xׇ?¶$Хϵ]?¢=Žwf?™ÀR"?êV#º:X(?¸U'
‡€½3FGL J2038.8-3613@"o›™NÀB5™€o&)À9§ßV<L·À;ªÍv?ø>¿¼'ZqKØØ@
@6Tû¯ä@•P?ÞgT¿ä'@Ö½o¿ã	F? ô¿éÛIq&ù¿ä×›¡KUNASNone?êxæý%¡²?ÂuݔýÀî?¥årϽ?©V¶òÙ¡?À£Wzs?À}Nž¼ÑB?.?ªz<`+?"õÂDÄ?"fª¤».?¢Ç¤ŒõÝ?¤!H³?ìH0â:J?¨B"ZƒÓ?£	€(/^~?VK†‡?¶XþdÖ~p?£±¿çא"?ëxEvÇî?­gg# ¤ô?˜´Èû¡ê?"'T4å†z?¾8*B
Ø?«†'죢3FGL J2039.7+1237@L¿/˜sÿ¬À12vd
k"À:`ýŸÓo~À;®QC¿rq¿õÃ{胷…@ò…¶Æ'@Ç«_ê¡I¿æ÷쌡¿í"ccÉöP?ÔÝ!yJf¿í˜[¿Õ~³UNASNone?î"è8jj?·a©è¯ò?a¯ßüi
?i½žQÜ?¬¶~rÈ7?·,Ò.£û}?ïŒ2Xè(ã?ZÖüìÍú?eNÞ¤ÑÁ?wÔÛæã4?‡ŸèÎL'i?šPñ›ª39?ê®Ï§2óK?©qâF¬…?³7…c¡‹? ӏQØ?·QýcKÄ?¢b,Ãä?îòÀ£×¨ž?¡ŠÞšV4í?~‰i3?06dÍ×? É¶¼@ïð?¡ˆs"23FGL J2042.3-5416@u{êüÎXÀBÞj㣨çÀ: jOÿò"À;¼àm"¿å±ÿ~GP@
¤ќj@lŠ I6¿â‰	Ú
¿ç"¡ì#¿éky˞¿ïû:%•»¿UNASNone?C ?Œ*m`Ÿ·?`"ÖíˆYY?dªóïõq´?ƒóêsÛÁ´?Š¼"n?îìØ?|5?¡1êìH¾?z#Ê!vÂ?‡÷èÆø›r?›Üˆ>»Ã?šßƒ Óܚ?íôŠ¸UüJ?•ùÁW­‹?KvZ8H
?‡Sl·¸Q?¢™M"Y?ˆWla?íÌ|&É;?¤œ	?O¼3?†ÿ
÷u²?ŠÄ]éjvÌ?´I»}
Çs?¢ˆá§Ö®3FGL J2043.6+0001@GNE^®âÀ8¸*º¾­OÀ:•sÔãòƒÀ;µ¤(hÔÖ?ëiG¡K·@
Ô爏Ü?ûÚ>ÐJ[?ÔSÙI:&?˜,Ɵ›˜ ?Èïx?Ï¿ãòJéÄe†UNASNone?î‹vF>–?¹j dZ?ÂP2ƒ¨?˜p`iŒ?¢Øž/u¸?µÌà×f…?îÒë–Ih?¢ß%ØÔï?…0'H³3?Œ;—ÀWm?›
y'y?R?œ‡¯Ü ¼?í~þCÄr?¡¢.ìo? ãÅ ÿTš?'_.?§,V¢¹Š¹?–4݌wU?í¯|j0
?ªí"Ìàz™?…óÁßú?''Í	Ò?¯‹Iõ;¤?©(ã~]e3FGL J2043.8-4801@uúw1ÅÀC!²_c<æÀ9¢îRX'hÀ;³ Œgï?ññ[!ŽÆ@|¶M"m8@ó‰à%¢¿åŸGŒí ¿Êx=3<B{¿æVH«•p¿ïÿÜ^o³UNASNone?Ð\t¤"ÐN?Æ5¤'â?㺞å2ˆF?ËD àclŠ?À\›">O?Áˆ:!?«TñàÞyÝ?±¶ï­¤«!?çy~²Ó"&?È?"43c'?ËDȼzò?Ä"Õs¸p'?ÙÜÀW÷‹ç?¶Ý䡯GÂ?Ú¤ô^nà?·"µ'£2?ÆþUgT
o?¬@ùÔ	×?¿ør{kžÜ?®±õyº<?éc¥iN3<?¶Ô›
­9?´êb:"ÇD?¦Ñ²oóÅ>3FGL J2044.0+1035@L)©~+VÀ32;yRÒ5À:r‰ŠWÝÀ;– f<tû?èݗÿÕQš@Fýo,Æ@S§`Ÿþ¿Æ
 œO#¿å¶ˆSåÊ¿ÙKY¥bЅ¿ïÿûC¾×ÓUNASNone?ïkv…4?¤æÓ@ø‡.?Œ\ÇRõ#?¢†ñ²ûh"?q‹.Íä"?ƒyµ27•Æ?íGT	ö7‰?³ê•ì$ò? ¶1ji?£ÛPZ	*?ªÔ´/2?«Bñ	fƒ?êl({™e?¬osèêB§?¸©²¬Œ6"?¤]j¸VÞ?³õ§–þL?¢ðU™­a?ë"±ÉŒæ©?®û@nê˜È?¢`%z+!r?œô²o«W?½º^öƒ:?ª!õ
µ3FGL J2045.6-6838@t`⡵ÇÎÀA¶Ü­¡À:kYnLÀ;¸à°¯_Ô?Äõ¿&,K@‰³*º=Ô@$¿²‡ý¿âú©/tóÙ¿ã'ú±À	£¿âê
ªþÆÅ¿ïÿóºÄ®éUNASNone?ïM½ašð?¢ÈÖÄ°ö"?gj¯ˆèþˆ?z؇Ë=|á?‰ÑäÅ_n?¡ÕoR>'B?ï;ƪþ?—·Á";¼"?wkñÙó֗?|:†õB²?™B¼­ªª?"·«+v•¥?í¿ŸÚÇ}b?›²ý'åÒ?¡ñ®×ðq=?'ßÄ0;ÖÛ?¢S{—¸?"{r,ÑõB?íÊ%ʶ/=?œ•ÐÅò?‡€Tªj?Rœ-«À?­}ƒrq˜?™ùÍ«h1j3FGL J2046.7-4259@vaŸ!-w2ÀCV4XÍÀ:mGÞ»ãÀ;Íw=N?(?Ö>éÜ°£@
ã͍@T kDò¿ç›s³¿×|žjÓwP¿×ƒ¤a–v¿è_¤]ö]óUNASNone?ïÃ3$¦Z?~³`:"c`?Raî3 S?Z;?z¨8?yÍò 1¾9?|M"Œ­?ï:ácð?–éFä
¢;?tæIQb‹œ?x²"/ݖÜ?˜¿‰Zß3?"w'ŽÜÙ?î'à· ú?"áׇ?@ѳO6?'«tù¯êM?ž€*‡³?ŒÐz®a?íùXìíy}?<mÀL}?€ÕN¸…7?z‡}êëA?¬d»ÝzF×?›b™ÎœAl3FGL J2047.9-3119@)©IÆónøÀB°>ž¡À9Äz•ÈSÁÀ;«zl­¨D?ê…ªÉÜq@RÊ/cšÚ@*zàEûb¿êþLÂY	¿á[_Ñïó¿ã"Åãà Ð¿Ü˛Lª±"UNASNone?ïYiô5Zè?š¿Ä‹ž~ê?u¼eXYÀé?€ÙQhæغ?ŽÇPF|ez?–)ŠfÝE`?î¹vèGù›?ªÕOšm"ý?€û•4n?æÐx{ü%? gҖ3>ü?¦K¼GêIB?ìêsl(3?¡õ®Žf˜?£þ¶q°Ñ?'C
sÆ?®TʇûË÷?˜ Ø
Šð?ìl¿ž"#Ñ?«õ(=³çÃ?˜–Ü]o?›àæÅ-'÷?¶•;f'Ê!?§Z]‰¢Ý¼3FGL J2053.1+6027@XV'Ìö¾8@$"òsPÀ9KŽÀøƒ4À;S"9-H8¿"ø¨ÀŒ°@&§}‡ë@W§Å¬¿ä¦!'ÕbÑ¿çÃOÍ¥¿¿è_¯ðjƒ#¿ä͚ŽGgUNASNone	?îòh nfÛ?«­ÞB[Ô?‰¨FD?•å΄º—Å?"ÞØñÝÜ?¨œj'~*3?ìîƒGÐq?º–+nÎ	?'îxÉõHz?–ynÏÿS$?´½³D*d?·€Oõ'Ù'?ìmC?—h?¦}¨–*?žŽdEðN?ŒÀªÁC‹?´ò_nIÈ®?¢@(÷ºwô?êž4FÆ?«yI¨Ú?•À»³¹Ï'?×¦²-?Âψp®÷?ªÈ[ÀLIc3FGL J2053.4-4052?íUÅߝ´ÜÀCä¦">jÀ:Yt^v­ÜÀ;Òù=¼¿Ä©ñÍڋI@4؃9Zë@TF__áè¿ä—I$_þ¿ß/.©9¸¿â†g1ßÃl¿ïÿÀtFEVUNASNone?îy/ƒe¼Z?¤Ã/Ï?‹ €͌f?ŽøÔ²¦•?¡¤çÄp×D? úP9ª2ç?î8'Dæóõ?¦éS†µåâ?Š\‡"ŸE?'¿ÌšœL?¥ß¹Ì˜Ù?¡f½¦)=?ê‡
"ê(v?«À!üO‰k?»5ªI?§ùEÙ?°'鎿-®?™r˜¿ReB?í…åÊ:??¢#h¦W?"ŠÅG'Ú?ŽhOê'?²™î	‰?Ÿ4XU$·Ž3FGL J2053.9+2922@RWâCV—À#»
QøXÀ9ÖV>Ðö'À;V±AV¥?óÙ£A«q@ŸÝq§?ø²€@LÜ¿á훨´â?ïþpßÍ@Ì?ÊGɉ1¨«¿Ùµíkí}¶UNASNone?áC£A†?ϪEŽî¸·?¡sïqv? [vª{P5?Û²úËN"?п…8¬Ù?ékWý×ç?Ë'NP©©?¦âV8]W?«,:Ù?Š?Æ*Ú
z‰?ÇeŽ¶ý70?å; Ô¾^¶?¶Í‰'Më?À靅­ï?§z
˜âû?Ê(a€×;?µ"Œ-äˆ?í
ÍÄF?³ðžüT‹_?¢6E;4?©ÌÌ?@8?­ê¤r‡™?¯,ã³m­3FGL J2054.3+6907@Zð¿\£@.Ÿ¾˜V£{À9ìÆ%鞕À;¤¡pþoÝ?Þ>ü³"	s@¶Š{C˜0@ªx z´Q¿ì8¦O¾ò¿—rÍËüøw¿í£­n¸š¿æ@²ôDÇUNASNone?ëPe}›H?À~­úÈá~?¿¨žm(JÉ?¿w»8&í?—PÖ§kkø? c†/m?許…jww?ÈùÑ¥™mÏ?ÃmÙFœ	?ÃçÑ#=ˆ?³ÞÁGt64?¶m²š…?엑œ—y?£úØö$ÀW?¦"òSH.Ó?•œô~Zx¸?°1úÉw,Î?žŠÏl¼‹x?ÝÄ(îÚu?Ĝ$âì\—?Ý*V+ؘ?ǙçzÃ3Ç?´FM•3Ï?©#á±úk3FGL J2054.8-4908@uâ'RT`ªÀD‹«`kÀ:?ø³o.À;¹wD;Ï¿ùAž‹EîÍ@P!ˆ¬6@ސ>&¿ê%£"˜ÅM¿çLèdi_¿ÎB×Ë®iµ¿ê"gƒqäõUNASNone?ïìY<°{?g ´ï‹±]?7¦Ô"V¶P?98æ–¤?`÷Ì?®3?e¢—h†)Ã?ï·Ikž­?}‡;T¼÷Ø?OH-n˜?Tý'þ!>a?€9"E,4?zæþõµð?î_ÍM¡ÙF?•Û¡Î¾àu?',{ÙÙ?Ut{ºy?¡mè_þª?í±1T?ì±H?…–	0:µê?Ý«&™7?¾úÑI1?Ç'(¥Ø5?…Ž›13pO3FGL J2055.6+1609@OlUÚ'(cÀ2KÈâ\
À:+òËdÀ;¢Y£àDy¿ó7‡mò÷¯@
‹fNJBº@ö_ÊëÌ¿ç
y]0¿éØyti¿â=Œ˜TJ/¿à\¢ÿã"SUNASNone?ï¡Yð΃?'F̸kÄ?97vÞ?@°î"Î÷^?†ßÖ ޏ?'è5ô)?率'øåî?‰d0PyŠ?_ò,ƒ?kݯ"Ò?'5ÕÅþö?…D`HÆH?íælÊÒ/?˜}º'èü?çŽj[¶å?ªÓ€C®?©*aþ%ž?" ÷OÁYç?ï6ía1=?Šþ‹Œk
?"M x6ƒ"?'¶§d—§}?˜ý¸‰k4?Šð¯~¯®^3FGL J2056.3-5925@u6;%oüÀCm'Èâ]À:*¤L{ÖÀ;áà'ód?ò'ål€Ü´@óùˆl '@ir"¢?¶rj5òµ¿ãDè›pšƒ¿æ¦üP¿ïÿÒ`_'5UNASNone?×ÿDªüh?ʖ•ÙˆÒŸ?ÛtãÑB=?Î!=O©u§?ɯȫƒ?ÇbÆ‰[l?Ã:KOÆc¬?¼4c{H2z?âLBexh?É;£†µô?ÑÊU+³X?Ä
Àëx
?Ýz*"8…à?¸V_Tk9Ï?ØW|ŠüÙ?·ï튤è(?Ä\±Á•AA?¬#³n¬O?Ì
D{&=?´wä9Ï4?䶤tî0?»|;"Ǭ?Á)´~.?®Ýt÷w'3FGL J2058.0+4347@U@dÜY2¿ó¬§
£3À8$óĈ[À:È	€²B?Ú¶óƒè#ã@݊µ%;@\¥ÀC|'¿ç;	XØݿ뎵jZ'Ç¿ïþh#¼?ï½IÓnãŸUNASNone?çð-î |Î?Í=—&w©r?µð[°nró?½´5‡øC?ÅGoFÓK?Ç¥d.‡EÞ?ÍRÖ¸Ž?Ò"~¨'s?¶ƒJRÒP?ÂÜ||ó—Ê?åçúǂ/?Ó
©£­c?Û(š†Ø
?·0㬽?ÇØ rcz'?®ý	ï¦w?Øë?ö@­?µv°¹¼?ë·¹Ëcî?óR±5=«?yNkDí®ü?—iË* î«?í¾«Ô?Ã}GUžÙê3FGL J2058.3+3729@T
™E¶ÃÀ†wc
ìRÀ90/JpfšÀ;;Ð<ÃÕ­?åðÑgñq@
ÝâÃJb@šåÀŽ¥ö¿íÀ°º¦L¿æz[>¦?+¿ÞèúÇÔ6ñ¿â]Àc÷	UNASNone	?íLÂkJã?²ïÅÉMü?'Oæ!º"D?'|òUY«<?±KPd7?°óÚ0°æ?Úûh=?Ò QX?ºo7*ü'?µ|»¯ö¡‰?ßkèÉø<ð?ÐLtIßcÝ?ê$ú~ב¾?«ŒS©?©¯é§ÁŽ?"ÈuˆMþ?Áš±Y!?¦þ-•iw?ç‹;í9ñ?¹z¶U¥'ï?¦ø§É°?¤u5]5À]?Î;ÑL¡%Ó?¸^ď€E3FGL J2059.9+2029@PÇQ'©"À0}°5½Q/À9öÚ˓À;…OºRvÅ¿ú&"î9.@hÛkv¹@œàŸ©¿ã²ÍN@ą¿ìr‹FÖº¿ßëtbS¿áÈAŽDUNASNone?ï
ßy÷"?£+òí;Ü ?T8'·Ä?ZMö&ÿ,?–eD˶?¢ã¹bCˆ®?ï"À¬ô?"é}ÆS?d,ÏÊæì?uçn߶†?†¡É{?<±Ìæêî?íb
¹>?¡6ù¢¶÷µ?"½#&?€ðêÁ}?²=¬ÉnÆ
?Å©Þ,a"?îˆyÒW´?™£boq7?"½&e³ŽÇ?)¶øÙh?§e¥´)1+?™›Ë.ZV3FGL J2100.6-7844@s£Á½¥À@W±B,Ë:À:vë»ÛÀ;¨¥º9LR¿Õè6W!qa@éÙM
Ð@Ú]ÿ—¸¿ëF|ˆ‰m¿èⰠě¦¿ãš&É\C½¿Ý"¤[OÃUNASNone?ïü|ïŠé?=LV«Ð"?‹¨¹??¡ãÁÃ?:™.Ueëá?:÷ÉÎqâ?ï²¢vÎ?Y9^Ëó›?S\Æ0&o?](='çÜ?
aQ_§Æ?~`ßZ?ï"¦›¤?†ÁÊO×ó?€"_Üg?m̬‰i	¾?–™™üq?ƒ5¸I"v?ïUË"Šh?ˆxÃʙâñ?3¡èXZpw?9E:ïÿ?"øŽ
I+?ˆSÎDõ"3FGL J2102.8+4704@V:§›ºÜ?Òë|eVFÀ9]»JÄIqÀ:üÅCk›?é/ÇÛ÷7/@ŠaÎQ1@'ÿ\—¿åև¶¼©¿ÈšUÅô¿ãQ˜ahÙ;¿â«RyÓYUNASNone?æBl»¬DD?ÈLÊ*K'?–užýÔgô?"‹pªlm?Ò̘Ê0ø?È
û°c³?ªÛ«>f«¦?»•Yt´e?³"9'~A?µ«\:ƒŒ¶?ëßÞéÍ"?«…*§‰ ?ç¡Õó<	¹?´ÿæf–x?±œžTéüd?Ÿ@'3A³?ȪYšÚç?±ÍH¬*'Ç?æQ±cóc?·@$'‰•O?°—>¤Ahô?¥Fò£å©?Îm›¿…?´ÐܐÊ×Æ3FGL J2104.7+2113@Q <K	êÀ0çr>á½À:\%ĵ§À;¤¬°Í"À¾|¥-Ì@Hÿœ'Ø@iÀÎO?ã߻зNG¿Õïãð!]¿èñ¾
‰"4¿­t4Cú6ÛUNASNone?ïÉ=¸_¼î?{>Ee©?f#•o@oô?l>KÜÿ‰?pOYQ;?t%ÁVØ^-?ïÆnHU(?~Žî±#Á@?R ¦ÈÔéo?XÚ@ÛS¥¢?x@²#6Ä_?{‡]ˆK»4?íÌú"ÏD?˜Gu²çà?ŸHëAô'?}—ö,ê<?£‹á6}?Œ',³¯ü?ï»I]iû²?"Ô¼Ç
>ô¼©â8W}?Ã{˜Ž0ë?#JP÷?'m›8êc3FGL J2107.1+2248@Q…£Â‡èÀ0V2.oÀ9ýE= óÀ;‡ÙRMI¿æå®Zk@
"÷P®ï@Ïã ¡5D¿æ–
ìZdX¿ç ^F~¶â¿è™•Rë'é¿×}‡TUNASNone?îrñ±
j?°gˊ~9?xɧ‰f¦?…
ÿ…Ý?¥Îkºh2´?­°.le}?ï‰AdV"F?•2!™Í¾E?gÈöµLg?xˆŠû—d?‡ìt¬­Û`?é¥.06?íŽÊµ¡?›ñx÷ŸN?–nŒ Ž?ƒM¬Á|I?¬
i/Ç?—0ð í/?îšIƒ3?–iø¯j?HÑHVa@ï?PsýÛX?¥û¦FsI
?–ŸU3FGL J2108.1+5202@WTów[@ÒÜʵ›À8n†º™ÄbÀ:³×û뿼« ÜrËé@/îWŒ@v7]d¿ßëŸTR¿êöò·åV~¿ä¦ª™q*»¿îݓ»Ö}UNASNone?Ö¨lX0G?ÉwÝèó¦ª?·²}üH£š?¶@=âh…Ž?âÜ
JÓj?Ì	jža?äP=:çc÷?͉€œµ­Å?ªEß0 ƒ?ªSÍáb>¥?ÔÎK$?ËB~žV^?Õ]È&a÷?¶õd!â<â?Ê{a¸î?°ÝŠ	A¤Œ?Ýd‡JZA"?ºwW¾ªÔÚ?Ýö&:wO?ºM±ìÐgÁ? Ï‰ó1¹?š*rãÅÈ?ßïÿH‡"{?»n¿'vÓ3FGL J2109.4+1437@OØ$>úèÀ5áŸâÚUÀ9NØ9¦ëÀ;"wÏDvÀ`Z"°ÔI@|p¿…¼m@ÜŸ‰Ê¿å>KïA¿ì²HČXá¿â"ÿ½ÿ™B¿æUÂ`ˆ7UNASNone?ïû
¥LŒÙ?^åüVR?å€÷ð‹?)¤ãL®Ñ?B—¾M''?]o_¥?Ž?ïÌbðè"=?xù=ý@îÜ?NÔø?Ô®?Uz±$×¢Ü?uóèxæà?v;ÇEÕ!œ?îó³«OŒ?‹ÊGe÷Ī?vRˆÃ=?e± bÏ1<?›ôæt	û"?Š¨kžÃí?ïéÿOiö?iš{ÈýAü>ºŒß_ÞÁ>Þø…‹+zÃ?eý^úûy?i—ãk]zŠ3FGL J2110.0+0442@Kx"ÄGÃ
À;Ö2.oÀ:;÷ƒY¼4À;³{ë2éa¿á&æxFä@³ªÎJP[@cŸâˆ÷¿à¸94
§¿åEø(<¬¿Ù
´ë?寿ګ贒vîUNASNone?ïô"·DO?Sfeb"°~?Q~D¼1?´ž36ÿ?V'¢±cº?Rô2ñ+Î?ï¾²!ö?{Óø'pø?R¹ÍSÂù?Vaw²»âÜ?|B3š€ÆÄ?yLǸ»æ"?ï@v!›4?ƒ*P_?}VmJâÇ	?v)ø˜»?› y懹?|}/^Ô?ï…	 ¿já?|¶°¿¿$?uÂÎ9? /p¢0<Ó?ŽŽ¬J‰H?|›°·0ñ3FGL J2110.4+5946@X-Œ*EN@Þ͍¼ì…À9W/ ×{|À;5(ö™Nñ?ÏM٘žX+@'Ë+·é¼@EKYl-¿çõ[s"x¿ïē_e7µ?ëçÖ4÷Ñ¿ìÊÒ @3ÄUNASNone?ê­×‡.°×?Âq+	XL$?–JGÔ
Û±?˜nC®·?ÂXèÁ/?Á®«	äU?é>X§oÅ??͑
§F?¤¨N|€F>?´KÏqÄk?Å܉à Ùq?ȳ!àJ¤ˆ?èpÚ¥3?°Í"¼"qŒ?¸QbBP™?¡¦JĹ ?Â2§æÔBé?©㎏â[?êfÑËH'?Æ]":#'T?lU"ì?'
¨Sþ¿K?ÅôK~­F?Æ>*î\3FGL J2115.2+1215@OM'#[NÛÀ8scä«æ£À:¯çÜôÀ;§Þ7X[â?×:m-n¼æ@6W'¸ÿ»@JN LO¿ã°Ì)Au¿é"Æ gƒ¿Ù¼%UÿÝJ{ñŠiUNASNone?ï|-œÇ®…?š'š»$?8¡tÔ§?LwÕä|äî?Ýá6ÜÁ?šXØuýû?ïo|ZöB?'ª×éú0?j*êÔr$?r.^؛¦¹?–cÝÍRø?Â¦zΑ?îvYÅêÜ?"èëgà)?‡÷M·•ïÛ?uVZw·'?¢œ3lÂq?Ì`ð²¼?îƒ'×"ß?›Mõã'?}?aLÏ2à­?h¤žî1ê®?­eš£ô?šÇ®?Ü×3FGL J2116.2+4422@Uél <K
À
=›l±À9ŠáçDòÀ;J¼¼´Q?ê¶çnþTH@
œÚ–Ž¢@ô÷í¿î°±A𪿿ӺãÒ^¿ç(þ'jöï¿Ñrž<W8UNASNone?è+½"ÿcê?ÅÁ½'*±1?ÆOxžö?ÂÃéÑàÙ¿?²Ôg×¢Â?´™D³®H?Ý¢‡J‰	?Ô° ÷֗?¸Aô¡ò›?¿ӄoç?ÜMePnúP?Ò«=ÃÙº#?èB/µ0?°i¡|ýoê?¸ueê;?¢—ô<ËÖ ?°†c¼JÁ?§V—óà?èár©Pì`?¿tª´?±Â	¶//)?´Òµ'Ôýž?Ù0¤¶î?¸žÒ3FGL J2116.9+1343@P	:¼"peÀ7Ü¢G'ÝÀ:/–WZZÀ;£æÎ-¿ü½¡'	Ó@ä–'IE@ØÍ¿àVôï^OÊ¿ã²íáx-¿á}-eeé¿ê™Š]ÅUNASNone?¶f¥?¤å§[S?pK§=ôb?‡WªŸâ%?¡Ù'¯Æ2¢?¢û(5æ(l?^?>'?Ž›
™=n?cϔFˆÙ}?r/¶yÅÔ?…§ƒ^Ž%;?‰3—Ë;?ëêP»Q?£‡ëž#‡?«¦ªæÉJ?–ÔFoƒlâ?²Úv҂t?š=Ƴ‰iu?îÃ>õÓË?˜—Á4z	z?>¼±¶?I 7Èw?£Ž?¿;Iã?˜s¹r#±Y3FGL J2118.3+5751@XcR?gôÜ@¥XÂ8õÀ9pËæÀ;d ;ë¿Ô³"î'̉@ÙM(§¾ö@Ýé_—e¿æf"suÿ¿èƒ¤ª™Ç¿ÞXœóg¿é)÷ŒáFÏUNASNone?íŒÁ%Ò3!?´Á]ªC6¢?",Èú–ä?ƒÓ‡jU?±]²Š{?³¡_Øc'?íYF#g#?´æ£ân?~[j·¦?'Àztk?³P;Â]ú?´ëq)-?ìÉÐk_Ó?¨£†êÀ? 5—ºçh=?1äL"ÿ«?·VåŸ1MN?¤DÜ –'?뀿þåF?ª0«K¦¤S?i`´€o?cޖ«É°?Á˜~/ži)?©ìèJÎè{3FGL J2120.4-1256@Cxéö©?ÀCmS?B5/À9Ô¢ç 5*À;µšTbX?äìwþÐfF@È'qßÁ@" ©ƒG¿âD4ҏµ¿ê*¯8¿æ"J®êu¿ïöEI5SUNASNone?ïä¦kß?gË~0YÉô?>Ÿœ<IÎF?A®ë\_æ)?g…ös
çb?f8¿K­=?î/%OlÞü?¤Ç|
Ø·?ŠJ^z²5?v9'£?¦{j'£·? mÎöhŸ-?îì*rS²5?‹%¨Ç³O?Ž´ÿ,4§L?|ú£ }m†?" 2oe¶?ƒñ¥ýˆ?ëÐ팮K?ª­1ú£Ò?£°rËüƒ®?"Óêy,}?º?-œKÓ?§ôÜA«
A3FGL J2121.5-8253@sXm›äÍuÀ?M>EþÀ9ð¹£$\×À;q©Ä[åÀåèô>×@
T"ÆK(r@¤S_ùdÛ¿æ!Á½"ã'¿è…sä˓‰¿àpÓþ"ù¿éÏÐøFUNASNone?í‡kÿ³]¾?µ:g"=ôm?dà?÷Ó(ñ?iq/~t£Æ?³ž¦x¾?´à;~ÃU?ï¹¥"ïm?€óöª9™?RtVØä"Ï?`AÉl7ÅÅ?~ RR"?}=UcKÕÛ?ì®ÖՆéÃ?£7V¹×o?eqTà9Y?‡ï_ÜÁ?³/ìþ£?Ÿ|ÀÉäì²?ïC±w.Ñ?š9¥÷Ž¹?läŸël}? ±ôW¯­!?ëÓ^Ê0=?š3dX*bž3FGL J2127.1-5615@u9EÁ?ÐÐÀEÎtŸM¡À:QéõÒ"À;ÇæÿëÀH•7µ#
@
ô6¯"'®@""¿æzšûÄ\¿é¥Ù	·¿Ò³:«ˆÀ•¿ïÿÁ£›G'UNASNone?ï\ûº?"^j‰ìV?@\…*bØ?MýGd'î»?‡¹`p^Ó®?"¿ŒRX?ïºz
>£?€C[ԁE?Md>Kg˜?W8Þ$Ät½?q°ó͸?}cŲV—?í$žãßh?r9æ×4
?¡ýhá^"µ?Ž¤(UUen?«¸¨à¯"»?–ˆ¢þ=²«?ïžÎǾµ8?Ž:%8‡¤>÷¸ßR	ò?ÁWÕ>ö?ˆ@q ©­'?Ž5ö¼.'3FGL J2127.5-6001@tê"ã¼Ó[ÀE:â–êÀ:Ç©Á/	ÙÀ<
œKû¿çš¼s°ž:@2"YŽ'©?ÿ5ºŸM¸›¿ç<íyÉ"¿Ï+@Ç+´J¿æú~˜®¯x¿Ìÿ)UNASNone?ïà÷%š¢î?z#£zÎr·?Oäg€Å`?\ߥFrk?gÀ…U e?w]0«Êï?ï•OðÈÛ¼?Åy#bŠ?\1ˑw¨\?qW'®§{?‡%Ê[šî?ˆêó?î«Ù ËW°?Œ<j.ˆ³œ?Žÿ:úËùV?~>óޖ;?›.i/
X?"2Lœž?ïléæàuµ?‡÷z£p"ñ?IàHά ?Sâ÷F?'"ÀÝ{èÅ?‡°"Da
ú3FGL J2130.4-4237@vgxÔýó¶ÀGWzÃë|»À9ŒíÀb[?À;©Äe©?ìGœÌ vå@•¼ÚçB@}´"9¼¿ãçÀ¡lh¿è"ïjÓÕÍ¿èý("Oý¼¿ïÿ¨óz÷UNASNone?ïû¶¨Œu‹?@»'3Xk?"®¿ç]té?!¤BQ<ý?8ó[¨¤í–?=׊RÇ9Z?ï´qñ"'
?€Àë"qáÏ?Pûó^à²à?WØÃÕ\È?€Ä/Cf]?~VÝ5Áøƒ?îÜI%ĞÙ?_ŠZ½X?'ïp"a>?'ê°;±?'‡j³
æB?'úL¿8Ÿ?ï"D=ÙN?ˆz÷Q{ç?U¦2#‹?]—‹GZ݋?ˆN{Ãyû)?‡z°ù¬q 3FGL J2131.1-6625@tjD›¥ãTÀD#")³úÀ9¦*Í3$À;Õ8¶*?òŽ1^FÝ4@©X†~߯@""_öŠ¶¿Ùî)òJhb¿ä¸pL¡ÌÌ¿éÔÑß8貿ïÿä•|¯UNASNone?ç†Hœo_z?ÇLâÁ7K&?̂"²­Y/?ÆX)¤?¥'ënT£¨?§ãb™ °N?Ø1ºøc1?Ŝ›ëžÆ3?Öi
‰·•š?ƌ'âö"3?Ñe7~C5?ÀÙêb'8?âǁY(¥s?·þÕË€¬?Óˆ
WzŒ?µ''ëý ƒ?½Õ
\ê;?¢7‰^"ã?ÙVT#Vfµ?¹
ÌAw¼?ޝ-"=)¬?¸û`"†?Àü'Øß=?°g3ʧ²í3FGL J2131.5+2605@S"wškP±À2F£"¯WÀ:)ë°½¢À;ƒŽÝ}ôø¿Û™Œ;Ê@óÝq	Øq@(¹_\±Ý?ï×*æ!va¿çÎk·mv¿åé{ÜÅ=a¿¶¿µÑ_búUNASNone?ïf­.M¢`?Ÿˆ€ÐR?b‡dH;l#?hœWúUÂ?Ùm­DF€?žÒ¬©StÒ?淚ێPv?'–SÞ{Á"?_feÐ&þÊ?k–á…\?'¯¼bgÅ?íÑZGó ?í+zeÛ¨?œ xbÊÞY?ŸvGðÑÛ?"Ç6Ažñ?­3˜ÜŒ?"œ;ä3–5?íø·-Ô¼P?¦jÎiïm?NØ,hô?X¸mC‹z®?¯ülóS‰\?¦R£á<ð3FGL J2133.6+2821@S£ëJwÀ1Q\éåâÀ:*`	UXÀ;›•]ʶr¿ñsp/g÷‹@¤ž™ˆ§¯@üɀ'±¿ã>úµ?	¿éòµht2¿ç–]Ê¿Ðô˜PæšUNASNone?ïàµZ€4Ý?L™4fŽ?MWùRJ–H?aYS¸OfW?gô§+8}?{eÍWIßY?ï®â¢Û3?‹FKáÊ?\[·©Ë?h²¼2¨D?€Ä+Ò>M?†µý;Ò
Ð?íÝs‡>Å?—M_Êþw?'œé¥&?½´ÉQÑ?¨ÚZ9‹)?"BO²Î9…?ï`Hö?ˆ›NÍÈÖ?©ü?'ƒ
àᥰ?"ámÊCgD?ˆåUw"3FGL J2134.5-2131@<ëÊû;u!ÀFŠœË}AtÀ9H£ÝÀ:À;¨jJ÷u¿ùñª—˜¸s@¥P+¼q`@`M¿Ø"9Ùô¿æaaÍX¿àâÍú–«ö¿Òéå,XèUNASNone?ï²fUÊ
?¤ ø\Ò@-?c@»w543? xᖪ?™Á›Æ`?šVegyv?﵌‡œX`?"êPÁÑê?Lµ@õ?U®}<¡X?€ÛÄèhh?ƒ­ø§»´÷?íêz¤ó?™Ú÷üìæW?–L›0´?†[»(ҁ?¦^"uE?"ÅXÎS?ï`Ë(ãŒd?‹kžÓÐÏ?>T苓Z?Z½I¹ça?"Ü{¹-Ÿ?‹fu%+3FGL J2135.6+5742@XÆÂÎFI@ҒwcåÀ9Zžˆã—À;ëóف¿®×¶Ý7®6@)nu©z@ÀôÌùî¿ça
ߤb¿îM:piI›¿Á.Õu½ÇK¿ÒA»X¨…UNASNone?îßÉ8 s?­'"ª&°'?GãÓa'o?JVuËþF?¡£Ý1ð¿?­lT¶f4Á?êÛÆÿ´¬±?Èä7ç'H?€D)Ÿº@Ÿ?ŠÂÉßw?Ì¡g1©1?È)¤Ò/˜s?ëöƒwn?­ÕÑTˆC?šß^ð¤Ñú?SÌÅ×}š?À_ÐG݈?«‰Œ"âN¥?í¿IÄî?¥b¦Í±÷?0r:ð¯p²?Acën¹?±õE6çܝ?¥`o:ÞòÞ3FGL J2138.2-4939@uÀE¡ÊÀƒÀGyÔbÃC·À:,õXQÀ;^ç$?âíÊ$"w@q†žj9@W*?nªÙ¿â¼V¹ä×t¿èª9G@Ô¿æ¼þ'"¿ïùÚmZ‡œUNASNone?ïžŲ¢?›îlsN1?zÐSú?€˜ƒ
öŸŒ?•x:tåB?˜'ƒ³	
?íz ˜'cœ?®/û'¨r?'yáłþ?"Ý!'D§Ê?¯•GH?¨ð‹™bµ?í3Åæe¾? H±f%Ä?¥oñíö's?"?dqù¹È?§_ñ³£|š?"ºÞ8Ÿ+?çEZ½×¨?²ê%eEýÏ?®‹hà¾Ì"? uŸ\Yr?ËHô\Øî9?±½ÜÚ¶e3FGL J2139.5+3919@UÐ?'æFñÀ#бx³pÀ9›ó÷´$À;}ý¬h©?ð¥\ürÖ@+ƶ³/î@ƒ¦¹Ù«¿ëÑâÔ1V¿å'Á³`Œ¿àª­<±¹¿ã>›¥ÂUNASNone	?ëþ®³Š÷´?¼ ¸à—›€?›ZÅnHè'? v)M,Rð?¹3Ù:?¸¯ÑI*Š?ãoÍS`Ô$?ÑàWÐGs¯?´]~ÁT.?µ*½Ê"@?Ô	9Ž¬?Î(ÓGÏ•?é¿	4N"?¬ûÿ2¼Ã?´uZÃCè?Î="½"
?¿Œ¬ó£\?¥ºªù[‹?èŸåî2?· [˜ÿ$›?±ß³\¢ý]?°/>,Q÷?В5õ¹?±ÓšØÇ3FGL J2142.6-2029@?$i@5z5ÀGG@Ý?á—À:å¡Ý4ùÝÀ;Ά"W£?ä¤õ߯lY@
Ö3=o!K?ø[6CÌÞ¿ÜàÃ2f§¿à"ð&½ü¿ïÿƒb½?ïÿH
úƒXUNASNone?ïƒÃcåµ?£aüþíd?fy6mGÜ«?r"Pz3?‰›Á‹´›¦?£$ÉÞÅè?ï™(ý1?žYÏA¯´Ñ?a#BšÉÎ^?†ž¹¯à¿?…r¥G½?•V(¬?ì¥"Ê©!?¢ÜZ¾<æ?ªÀ®£l7?œ£ì_0¨?ªî8²»?—_ô§mÅ3?ïe(žžÁ?¥.³˜JÐ?a½Cqʚ˜?†P¢ú?š;²}òԘ?¤b˜Ä¬#ª3FGL J2142.7+1957@Rnì€Ç:½À8dv}4ßÀ:±<¼M#À;ÝGP ©Ä¿âjaj©9@
Ü7ùÁx@ÆÿXeG¿î(ÂX¿Þÿhd‡,ô?Æ;4}¸	¿çxšö]UNASNone?ï۵桻?žh±wÌà?N¹yR'?"ض¢?lÈ«& +?"&—mã~-?ï›Ê¸(u?†]­vÖº?ao¨ÓòÏ?d‹~£hP?"±gÁ ÀC?ƒ¿……}!?îáJ_"¤º?‹»Ú
:mT?†‹'†×˜Ñ?x–(ëêa?˜êÉÿœ-?"CXjWb÷?ïage²"?'R׬as?*·{Ï¢:ì?;/t–?œ?"­»ªi?ÑV-G3FGL J2144.6-5640@u8}¿HÀFßÓÃa@À:œF&Tþ_À;¹ÌÏQ‹?êÔ¥ý¼?@až½c£@¨j¥§š¿ë'FcM¿ìdG"EL?¸YØxýlÓ¿Æ\Z®î"UNASNone?ïéî¤épì?ju™ó'Ú?4Xº$e"?<"œclÄ?c†CÒ‡†?iC™	I?ï‹x7ú–œ?"%êãx?^:hn*Lò?yÀ0©×—?‰Z¤ó•¨?¤3_DMq?íŸõaL}´?š€J°e?˜Å™Œ"€ò?Š~ן÷<L?©Ý$õä1?"'£ø3?îQc7\‰?¨¶,¨×¥?Wδ½%?wAj 'F?ª+°—?¨yd§c3FGL J2144.6+6606@Za¼@ŽÉ@#ˆdüÀ9Óz¬nˆtÀ;ŠÎû{6ÀQ*3d>@7å´™@¤ÿŸÝÖ_¿èz^ò\¿æ¥6û꜖¿ê‰Q"Eä*¿³Ô~.õ…UNASNone?î;Õ"‡V1?°<²'ËÄð?ü=ª´¼b?†?z\¿Ð?§ÃžlÝmÛ?®¶î†¤Ó?î˜Rß0Ï£?²ZˆÌÒdˆ?jäÌk˜¶Ž?ƒd«tÿÕÀ?¤Ì…F9z^?±§-Š±?ëì"œ	ŸË?©J «ÚÍf? "¨¯Èe
?Çðÿ:ì?¸–ÇÎÏ?¥©]ÔMé¹?ï‰_Ž'¯'?‰Ö‰Ã¶€>äpëÉNàò>ûòÔ©Õ5¸?£ ¡ÇÊ?‰Õ0"ÚY3FGL J2145.5+1007@Pƒ:'£À?‰Å«âqÀ:žÉã%ÕÀ;ºF"
q?ØøšJŸ@
%Â4‰´?ø××?A‰b¿ïĸ#G'Ë?èF"y&²q?´pUñÍ¿ºî‰FKz
UNASNone?ïòw]WŠl?b¤'iæ¯
?!«»KxT©?$Û¯5R'?XÛÍç|Ì?b+ %ô´ò?ï­SHí¸?ƒi»S©©ø?V‡¼2¤¦?`©ªWît·?ÚB'r}]?»—U"s?îîЍâ9-?‰,¥É‡?ƒºÆ žŠ?u%WÍǟ?˜H‹3i•X?…'F+#õý?ï™á´À|"?ŒÕ?¢\2?K´ø…2G°?]<®(àR°?‡ÌCG¶˜?Œx¢JeÎ?3FGL J2147.2+4730c@Wnõs}¦Àk¢æIvÀ9"La…VÀ;6É5h—™?ãÓä(^@
Vu´¶@w‹¿ç60¿â(ÙcÅ2‹¿åûhk¤=â¿è¢'ð'ßn¿ïþŠ¿·¡UNASNone8?Þ¼×xü?Ç·~¢ÂÞ?ÄaPñ?¼ÛÇÑ°?×aÈÿy?Ƽ 2îˆI?¼->ƒ;?¿w'O"y?Õá<#ÀßB?ÃÉ;í^?á‰Áª÷¿ø?ÆO[n^CC?æ'R|uºô?°hº³•6?¿×·½  ?¢õHrî…Ï?ÅÊډʃá?¨ãŠÖ+ß#?֘ä;²A"?²Omê}8?ԝíÉlá?·mÿ§—Q?ÔÉ.®"QŠ?´QŒå>"ß3FGL J2150.5-1754@AѺ^5?}ÀGºCªy»®À9¯[¿PãÀ;¸@p"Í¿¿J‡C3d@\>ø8`o@Evå¿èFì‡'Q¿ìÜìÌéË¿ÜMÓ4<j¿é	¿ônž¼UNASNone?ïÞµšôÄ)?u§@0ó1??®¥ÑE?FaR·´ev?mT¡ÇçL?s­Ìb®S?ïmÊjFe}?;	@
?aGd+
'¶?fž›èƒð?Æ1Ñ«H?ÓæYF?îÊmÝR%/?ŽxŠP~?Â,Æá6?u"-†ƒÅÜ?Ñ-òJ¿!?Š˜!%ýœ¶?îEsÕÞÕ?šH}¢û‹z?YS¹‰3±?Vö©ýÕ?ªå*öY±?™þTO]3FGL J2151.6+4154@V­ó¶E¡ËÀ"åÈ23XóÀ9°ÏS(œÀ;jV9Èxª?ç;™|Ïo¦@(ZÅ4¨?ý"ˆ`Xy?ïÅÛýþYH?Á7†""0ý¿áö7™¿Ñ—ÔtAUNASNone?îA¦J"=?±Â¢Þ.8ð?0&>Bq?—Ê—y(i?¦Ä'Ç+?®z¡Úܧ?ê<K\½7q?É=7á–Þ?¦"¢…Mÿ?±ɗÅU?Á†)ë·¢}?ÿ2ojl¨?ì­æÌ ? ·"ÂZ^Ó?¢ã$náΡ?‰tT/,?±=¯À·°?™]X»6â?åµÃ)îû"?À‰ÀN%G†?ÂDñ83æ3?½ºŠ?O%÷?Æä +ƒ?¸¦=OHfÀ3FGL J2153.9+6626@Zž†ƒ<`@"ÚÚUK‹ðÀ9²Š½]ÄÀ;%ôß:›¿Ù]W…3A\@–"t¼@5_®ç4?źÚ
fпàWågÎE¿îÀ°^×ý?¯#³=£‡UNASNone?ê´í2ߞ?ÂWÇ í?½˜×ÙYŽá?Àñ¬Î˜?©wzèT?² ‰‹¦ñ&?íÉç[Ò\×?·; ;3)?€­¾-,xO?KùC'a=?¯6·y?´Y3—Ê*ú?é3çȽú?¯Üå&ä҄?²í07? e^ÐpN?Á¹ÒRÈÓ?«EÏ#·	;?í
šo¤›?°Œ_çXæç?qÁ"y–Ö ?(M\È&?¶;A¹È?°ZÓÍ]wH3FGL J2200.0-6930@tö"Fs'ÀD{ꁺÀ9°Úx†ú[À;À‡»JÄI¿Ýjá€Õ@
µ"}¥ó@Î
Ÿ–2Ý¿éŽýCô¿à7ðeiwy¿éÛ(I+¿ì9Š¹	ªUNASNone?åȍzœ?Çãšæ¸?ȸ^ê'?Âcud‰Ás?À
k†Òý?¾«¿"LÕ ?íNœrݱl?´Õ˜~1÷?–€\*æy9?¡ûm¾ü?¯Ö
¼±¬±?­ÿ­Võy?éəª$ˆª?¬B¯Tˆ?»wÃÿ/?£®öÄÀ/P?¶šºêܜ}? ƒ·Á?ë}2)•VV?°B:yÁ®?£íTÑ?¢ÙçZø¡ò?º¦<«Bç?©;N
¦3FGL J2205.9-4704@uàÛv³¼ÀJ•=êFZÀ:RhDŒ÷ËÀ;ç&p­F?㋖͝"_@
¡rŒÖ@OÀ A¿ì@%"0›v¿çÿ–VKÄ­¿Ô›ã<óå¿ê??\¦
	UNASNone?ïÎãyä!?yÿc–Øu}?S@‡ï´?X]ˆ"Œ_?s®sP'T?wxWëŠpõ?î=¤^–?®Åj&'F?'߻þÙ?"pTk-®?¨‡vfÉ&ì?¨?­'?í:[P«Q?žÅ×½ŒÄ?œ¸Om»B?‰ü»
"¼?­þ=Ð.mR?—Ì£çòW?ìé"ëó?±H»@¥?—IÛHC?˜ð~,œ?¹K¡ÎZ?¯O)Äœ3FGL J2209.0+3652@V5*"8	À.ûBªŸ{[À9Ýã‹U38À;ª€÷â$M?Ä*½ðs@
¦zÐ֜¯@±Ø@žUÁ¿éùö˛@Û¿íÈnµ%¢¿É$ŒÅSd_¿ß&Yÿ»UNASNone?ï›
FZfÛ?qRkJôÞ?Oç؟£)±?T\€b
"É?‡>0ßlj?ŽUùù¥œ?îÛ,ê'û?²0¥ÍÉr1?=#eëÓ?"X±ñŒ(?œD
ª?¬{®k]aj?íf/·Ëæ? Å#3™ô?'ï~_í?€€›y(¦?°R»ha¥?œ¡ðéÛ?íÛºé`"Â?¥×˜Àv6Œ?`"cŠÈa×?jÂ{)È¥?°¡˜¨¦ä?¥ªþ;iØI3FGL J2209.8-0450@K׺Âß
AÀFÇvõ׈À:--U£ "À;eÁsÓ6s?çÒR:èç¾@]ûÞ³)?ôA»¿3\#¿"¨ÚúîæV¿ã¾6ÿæX(këÔ?¶÷›CÈÆUNASNone?ìX³×,‡i?ÀF¨ñ×<?Q@ŠÀ[?] E"ÕÕ?¼õa8s¥°?ÀG(÷©¡Ê?ï¯A'ÀáC?‰'4òkw?Rñáoð?pl|Ž®8è?ì±‹˜?"ðR8zŒ?ìkrY"÷Û?¥?¡#™?­*LŠçÁ? 'ÍÍDþK?¬ãÁš˜?›«óM4é?íSãϏM?²Š£}?^ÀüÁgå?q(m‡#?´èzƒ0ÿ?±ø>'WŸ3FGL J2210.1+5925@YëäO QD@Àc'†WÀ8œzšÐÑ>À:æRxrØe?ìÌ;5œUG@0–Jښ@üVàŒr?¿á¸VCT¿éF'ì‹¿í¤ˆ3{闿îIšt¤±jUNASNone?á큡Ë7ñ?'˜ʶ?Ò?q©Ald?Èòó ·´?ÃË&PGs?ÁPd¦ðŽ|?Ê­ý;$1?Ça=½r?ÔNØp܏?ÈTž7?ޥА†VY?Ìlm"é?Ù°ÏN{ž?¸ªIº"?Îƺ3IÒ¢?®æ‹ë|"?Öì‰›?¶i{®Ti
?Å2–Ö3Ø?®ó»(÷ÿä?݀$ygbþ?"?eq1|?×搀­ƒ?¿«W^úË3FGL J2210.1+6043@Z=îx@@AéÿãzŽÀ9Ë…ãpÀ:Ö8Ûé B?ÕÛNt®@gAžÛÍÇ@´ò€e–¿çý%ôËj¿ïÿíb»ÙW?ïüÎδü¿Ñ$|bßUNASNone?áÙj>;/Ù?ÑaˆªhW,?q'Rç!ð?|;Œkji?܏>Å?Ñd|¡nqó?êŠ\œQ¡¹?Î;yRDÇ?€_œÿ7»?C ¸ü:?ÄГ¾Åýi?ÍBÊ}B|…?ãG¼pË­P?ºŠ
u?°DRÿ"?¡ïe£š"È?Õh¶Så~?º38l!ܵ?ê©Û'L9?ǺŽ†Î?+†…‰DV½?Sh°€v—;?ÅQ²LT~?ǺBI3FGL J2210.2+6509@ZÁøL­W¼@–*"Š>À9ƒžòžîmÀ:̍Wk÷ ?Ú¿Ýs–®5@áQ•sð@ϧŬ¿è'+f¾®…¿ëŽ´Ô©˜¿ç""
Ó2¿ÂÆ!{¿'ÑUNASNone?â*—©°Í?ΔúÌãl?ŸJðŠë
?¢ù•¿jÊÛ?Ù¶1g£ïµ?Ξ{¬?ëOßøç®?ÅäÎe#+A?‰^¦¡ÃĬ?˜<Œ\ъ;?Á*™r$ü?Äf&n'ˆ?â'
<NÖ[?·†§Ck‡?·íª¨7Ÿ²?¦7"TEj3?Ôâ€ÝTk\?µø}΁°X?ç7î•ì?Â,û¹˜iÖ?}(DAyß?ˆ8à]ߋ²?хNïË?ÂôoöŸ53FGL J2215.5+6122@ZV~ùÛ"Ñ@™l?Ä;.À9Ó'YáÀ:Ég¦†é?òíȀþç@
Q[ÅM§~@;¿Ý/ñ¿Ò±kã(þ¿çèFiµ•¿ë…ü~ ¨¿å'ph]¯UNASNone?¨²±‡Pû?§ûf>Ý?Ñ.(É°ˆ§?Ê­Lv1?åÝÀ'¯Æ?ËÒ ÄzÒ?Ö.rg?ÐìibPw7?ÃÅ(Nk?ÁiÔÆK^?ßîÎfÈWX?ÎHò\4…?ÖP¾s­¯»?´®
Ü?ʎÚˁ?¯BÛK?ÜgÔ}Hj"?·4µGDJ?Ƒaߓ|-?³"lu2L|?ÕÉÅ'43?Åz§aI\?ߝ…K
¶?ÁÙ­—ª»
3FGL J2217.2+6346@Z·#c²W@KpïVd'À92ÀÁ%ϝÀ:ïµk‡7—?ÙÒ
	ª^õ@
>>lLYu@v/ŸTïq¿ÁøÄË)<B¿èîaœýý¿å¨øál…Ô¿ãS'æ&]UNASNone?Ø2·o¯í?ɱFÊ?/ï?¸q.S;·F?¹x"¾",?àØ~}À'P?Ì;1gú•"?äEóݸ3?ÐΐÄï¯?£v<¨Ýfo?¥Úª_֕?ÕP¯t0Ë?Î
$×zh?ã–óÖPF?·ºª%Òi?¹p!í[!?¦b–TÞK?Ófɜü{n?µÿjüŒ"?àäbۆNc?·Æτ9ԓ?¥ì`'mà?Nu ÿ?Ûy®6¥À~?·ÍY»Q æ3FGL J2217.8+3207@V3RÒ4ëšÀ4_¢œwškÀ:Jß72œ4À;Æ|°TÇ¿ê©ù>a˜@¬Äĕ›³@(_o§-¿åØû)xí¿åÛr…¿®<¿æcY·_ü¿â*Ûì'þ*UNASNone?ïhßáKÁ?Š¯Ö»G…?i±ªÍz¼?rF#>R¤,?'9]c¹±X?†È³ïg—?ï/4ÚÄ>ú?£À»Wz%?y"‹ xyÞ?UišG?"´ßZ5?#|ó^ÿ?íÝõӔ|?–´Œö-Ÿd?"ß,E‡Á?'ÙÞwzÿÑ?§±£úg¶?'%fYrµ›?î=;Àç?š®ß–š<Ð?a]0A?ajØ&çÓ?«v~΍?š^%ewºf3FGL J2220.6-6833@t»ƒÏ,ùÀE~s>»ýrÀ:p'Á—åÀ;úIŽ¿K?Á3ÎCoks@UQŽ&ô@
`V,?¼ôty­¹¿¿#H¼SÐ.¿ä­>!MØ{¿âiØd
NPUNASNone?ïîGÔ¤ï‹?`¥0²Xp¿?Q
¾ÌKäm?YŒ›"Ë)?Rb—éÕw?PŠì÷¿[_?ï'Ò?ŠÒ¨ýØÄÐ?`¢ì{ÅG?d—!®¨:.?‹DQÄàK
?ˆ,q?î¸4›¶ðº?Ž\CÐN%8?'ødcßÍ9?…ƱÀsÿ>?–%B—?€kJÆôò[?ï‰$Y¶?'ŠÅLè?y(1åE6=?tÊ*<ð?˜äÎû‹È?Ä™ŠÖ/Y3FGL J2223.3+0103@PMÔA5TvÀFL\|ؙÀ:>}—ÛSxÀ;­?)
»E?ÌÀ™~§â@
Ñìšó`à?üðxá=G3?ŗÊeÙ˜¿á½'œ¹Î¿¯"ç<Ü÷Š¿Þçg¾çB*UNASNone?ï½8öE$!?ˆä—fŒf?6m³o¬‰?>Z?"šV?ü©¦}Ôß?ˆ©r&Øùb?ï"ʾ‰ó?†³ÄþÂ?Wö,coòo?^q´ÅN]Ë?‡ÎŠÑ:ú?"9ˆ:¹?îÕíÙZ?‰¯À?´N?ˆ`0és?v[@ÈÎô?™:EJ:à?ƒû>SÝuz?Òy?Ÿ2¼§ë?QÞ
9ßË?[ÊHFÈç0?¯`ç#é	p?žà!¬<Û+3FGL J2224.4+0351@QšmÚÏÀEsG0@9¬À:sˆ¾€À;§¤&»U¬¿É'6G~ˆ‹@HtÓ¼€#?ù‡µ'm,?ïü6Ìq'¿àà~~ú˧¿áÿx÷žÄ?Ĩ0A\ŽUNASNone?ïÖUeî9?vßÜ7Ç%?)°•åzæ?)	0º±l?tÈYÌw¢?v®µ·¼Oü?ï½ïºD2?}˜íû¼‹n?JŽdÛ°5ø?TË?%ED?}¶Vçßþ?{e*0ô"?îo#¢UÙ:?'µm-È7?')馌Ãç?"q}Oôãï?Ÿñ¢¸Ë?‰y»£˜Ç?îǤ¦Xi?"Ñë"¡?9/G!ÁÉ?M¾ù3]"?£SW¸oÚ?€2'Ó3FGL J2228.5-1636@Ew}XÀK®ðà¨KäÀ:&êÓ²šÀ;¾Îf*…?ã'ó¬Nkã@<k›"€X@
Y ,Æ2¿ê£Oÿ'蹿äDn[¿å^gæ‡ø¡¿Ú·ï-}oJUNASNone?ïè$Œö1©?jö‰ÎŸDÍ?LŸY¤ïv?R"MxÛS?`³œ 'y½?e¬¶ˆ}÷?ïžç?ŒÔCâ-?[^ïR§A?küÓ(Ód?"äÑ"ë??ˆ"«èÔVë?îœ-4*¸¦?ad€zþz?…ãCc±%?|–žÉ­¸?·gØ÷É?ˆ_Ï«N_?î6
XÆ\?ž0UéÒu;?u6uÉ?}¡"q7?©ølkºxs?œX ז3FGL J2229.1+2255@UB>ÕÀ=FژgjrÀ:9^>y¸SÀ;ÊPg÷`¿ÎnÝ	@Oðò'@é®@o±¿¿åüCà‡¿ãù!3¶¿és¤¦©M¿®µÎCõl6UNASNone?ïsXê>ÝÃ?—Jn¦	€f?oŒ)ÖZ¤#?v†êxàÛ?‹Fºú±æ{?• ×¥N?ï¡m"YÁ?Ž›j˜¦[Ê?]=)"é³?kÚ¿7aû?"ÿyW±?Š'ò®ý©Ó?î j²åÐ?–­\ƒé?"1ƒµJu‰?ƒ[üO*N?£à'öýÅ?'
ô#/›?ïHK]•
\?"ôՙX?En'¤ŠZ%?RäµÖQ8?–K#:£?Žé€†'Ü3FGL J2237.5-8326@s3"µÜÆ?À@DÈ`VíÀ9¥"L["fÀ;6dÃÎ÷?àŸñgêR¢@¾æåÒ­7@x4€3>¿çð¥ë>.¿â5v{Ô¯¿æûFf…‰Ü¿îVP.@°UNASNone?éI¨s?ÁSí<©‹R?ņ{ýüJ!?¿ã¦-½LY?¥L?V$P]?¦´IŽ?î™ÍšÉh?§~—Sñä?ŽQC[†/;?'!u¼'¡?¦'OqÝ·?¢Õþ9Ø-?é"÷<Áº?°¾
f‰ßÞ?ÁG'¿Š?ªTÔ$ÍÞ?´¬RÇêÞ?øÞʦpê?åëV¬Lì?²…ªAøV
?°hJê?ždÃt;?Ð@xbë¤?±F}ŠÛ´3FGL J2244.6+2503@Vpڐî¢À=ˆb¡µÇÎÀ:§x+ŠÈÀ;æ<³åu?éÉÇè?!²@
Õíðˆéž?þ¶1_žv"?Ü*Ž'?µO˜©
¤¿ÕQ:í^45¿à¢Ou´7UNASNone?ïØmL˅á?tܝôV¾?QœÎ¢›¸š?V¼L±H?nÄKã,A·?rD­jô÷?îöyŨ? \¨Þ^˜±?€=†{¡Ê?ƒÏ—%?$?™	Þz'?šPÒ÷û£?îiò^áì?–+¥}ó²?"'Ë}ˆ_?†9#–µæ?Ÿ/è¦Wƒ?Ô$rðQ?íLJã\?£ŸSs ê™?™½×ê»p3?–S; Ê4V?¦¨•Ø̇ï?82nÕý3FGL J2247.2-0004@QÂÀð ÀHÞbäѦÀ9åóìÌÀ;›z6'?Ëøòd•x@	E—丧@Ü·àð?¿b v°¿æûÒp¥¿àÞ+ÿ7X¿à,_ÃEJÉUNASNone?ï´DVO?'ŠiцN/?HÀ8ƀ»?Gv;1Û½?býÞ7?ØGÊN?ïƒóL'h?‹âf£eõ?^‹|2©Ht?bʤRᯉ?‹f"¦†|Ë?‰¡ºb9?îjUÏ?"îdL?uß13µ/?=㈾›Z?¡¿y4þ?Œ=û	~Íâ?ì»zØJZ?¤Ç¹D½KŒ?oASìb͓?o'ãsv
©?¹* *–Å?¤|½²@ª3FGL J2249.3-5943@tqŒ½D¦ÀI¥¶…ì>À:åwo£&
À<'Y
]QÀè>WÔ}E@
ŠÓÒO˜š@dhÀí_¿æ;Ïl—á¿ÖËÑǀ¿êêu'°"S?ÈKÕI%ÁcUNASNone?îÚ±—ÐV?µ'½U£Å? …ÿ~A;?´ÐÿÖZ"D?qË@¸%ËR?}ÎôÈp?ïËëüñ¾9?x,o@äB?DuÑß̄?OÝx¬TO?wzÌäê?v•.ò©S?í·.SB£©?››3-ÂÖ?¢=_^¢CÛ?—KiM&?¢O»m3¢?h(×¹;S?ïõjƒÕá‹?X®²Hk$À>ÉM¶¿q"¶>äÄmŸG%?UQxÝ1D?X¬XÂ{æ3FGL J2250.3+1747@U–ª:э&ÀB*R¤ À95Õ"äFÀ:ë°Š`A¿×¡³†!9-@ݽ=¸@@H)`vP¿ê¹ý¯:7+¿æ~@–âÉÓ¿îìbïŽmÁ?á8¶ªCUNASNone?ïò‡sÿ3?f&õå¯ßØ?'q`¹Zð?1=¼€Ÿ4?X›Ö9Ñ?eWõK¼C:?ïÅÑÒLý?zþäE%Ê?G°ë¢mýè?QI}FÕ?z ùejAÑ?xÑv°TO?ë‡ÖWuœ?®ëkÊâƄ?¡Q⦌Ðy?—Syݾ?»ùýêâ?©^CœÂ?ï›à‹³F?ŠF3•ÔYè>ú"êp­/?"ck€''?ˆúšž BÜ?ŠCõ_ÿ)3FGL J2250.6+3308@WêÝëÙÀ7AÐúX÷À9ø8¢Þ¼¹À;Åß3מ?ó3¥^sÓ·@
êr$4¾@ÕãÿÄEë?ÜdR5¾)¿æ>k‹nó¿éΏ¿Q¿ïÿÙUNASNone?Ûnj³äÕ?ÌZúXD'd?Ôƽ%¹ÐÍ?ËÈ,‰z)?ϕ±‹$"º?ƽ£#fx?ÁU"Ûݲ¾?¾Þ4 ¤?åÛ8Á3Lg?Å(ú€ë?Ç=úU¤?»ÔÙX´ÝW?ßn©WÃÚD?´ù»nßÞj?ÖdS5?´:C—Õá'?ÄZH5?§˜ÞZá?ê†cl‹?¯ääHK²É?çI¶(j³-?¸P%ŸQ?¾]AõÒ=…?°ésu‡3FGL J2253.1-1237@K\bõ˜ñÀMb"aùðÀ:$tÎÀ;ÖËÒÑɌ?îy‡ôom@¥Ô/^@‰åÿά̿ØeöÕ¿èud¤«µ¿ç1ÉÓ7
ø¿ïÁRÿx¾UNASNone?ìñ}
;1
?µ Í'Èø"?§…¶ÜÜ»?¬4Ý ?©bxOp4Y?¬°u³ß¨?çõäåè·Æ?Â^Ëϗ/?¼ÁþŽq¾a?µ¥'.DŒ?ÁÇm!$Aº?¹ ­M1?éY4¥J D?¯ñAZ©?¿\\3oË?§-sœÖ6Ý?µÙþ¢;ã?Ÿ€—ccIã?â¨N‰ËAþ?µeBñ:¢?ËëYz ö?²0«'¢‹?Ésl;X×?±A?8SÓ`3FGL J2254.1+6229@[v"8…
@ ݂ýuâÀ8ÈI°M:EÀ;Gckà#?ÜÉhÚ	 e@A⹞ß@}_Ò"¢¿áßZËuU¿éö¾á¿é#Y…ú¢À¿ç§2ŋKUNASNone?î<Èó¥™?®žTpaÜ?gKfd"Ï?—ŠÊ"çΦ?£ÿËt%¯?ª£#¬yb?å´Xäý?˅¨C֍?¨Æ¢zìÎ3?ªÉ†Uy??Ñ~yèxl4?É& £V3ø?ç᎘(´|?²ñl¢Jê?±øàä?Ÿo‹ð薨?Ç}¸/P¼?®ë(zkÊ8?ãjî»9Ð?´)º1q°Þ?°(
ñ{ï?£Å›¼l?Õ"Ù¿Í-e?´M—êX3FGL J2254.6+4253@YM†DR?hÀ."'›ØÀ9µr҅srÀ;"=?%¯½?àFqï0¤ã@ލz&@FHö…X¿æ]ÓèŸç¿ç`XUŠ(Á¿éèx'{M‡¿ïÿ–ȦCîUNASNone?ïuÓyÙK®?''â¼C?~±ÄF,ܗ?…îó@B?ƒ2?f–¦8?ˆ¯g๨?ç¡Ã$"!
?ž¬ª
n^?ÀiϽ•Tº?·Ú¸À?Á#°'?¼ÎœÒ§€g?ì"	÷¬-?£
ÉnßÍÞ?©¸˜VÇ)¹?"nvÿ¬Š¢?­×I¾?™Ú#˜úP?ãÊ·äò–w?´9X
£>z?ɹ«·3ÁÐ?²86"Ì?ÇtµäV?¯HÓKz¥3FGL J2258.2-3645@8R÷ô˜ÄÀP$³=¯ŽÀ:¿Â"À;ïìì'(¿²œN˜lÝ@29Ÿˆñ×?ÿKA¿½ð'¿ãá•5¶C?Àe[é«f¿îÃnšµ?è«é‡ˆÊUNASNone?ï›Lo˜Z¬?—mü°Ûï·?ruù;€?'Hå«Mw?€#)l·?"Z²Îrþ¨?ïÂÎg˖ò?©·lJ¹¼?JÞÉÂÛ?ck]–²Ë+?{Vp@üE­?9aàÒÃv?í͙›¨5¤?™"$8âš?ššù®ëó?°æ¼{:‰?¥Øénx¯È?"(Nˆ,ˆœ?ï±zëé­1?ˆo™¨³9?N¡#Ú9(?hÑJC6e8?ÀÊóWJ?‡>cáXÙß3FGL J2258.8+2437@W.~ùÛ"ÑÀ?­W¼xÀ:ÈB#'À;š‰;}"¿ñœÝø©Ê@¥n‰ }9@xO #¶é¿ä¶_ ˆÿ¿îŽ:üçX?ÌÕp'î¿çQù¶©UNASNone?ïåpéâ.?'bJ*®X?$²C%lò3?]KÚÊ?iCñëz V?~éÞ?ùæ+?ï¾QÅÚÝâ?{¢¢ÌÔ6>?PT#¢:Ì~?VT•ÑV©;?|Â*[¾?x¿¿@Â?î¥vAU?'¦ÿ.€O?£3RWº?qï0ZŽ?¡?Ò·T¿Ó?Žæ'B9?ïk	ÔÍ?Õ¤—Upˆ>ô‹ï|Á?
™.;6­t?'™¢j}š?ÔŠ=Hv 3FGL J2259.9-1553@IXÜìÀNëD$>ûÀ:O&ËEäÀ;ãpûÞ´?çrÝæƒ4Ü@&î'm¦!@å®À>•¿ÞÏ
Ž¿à>íÚ?¿â"%¸«¿è*‡= UNASNone?ïNàŸwç?"yqÙÆLÎ?k†ê2,u¦?j˜â¿ª?'³
eËtQ?'"/k׃?î¼Y^í?¢-7[6~?¿XR6d?"üœ¡ý+?Ÿ•Wˆ'B?ž|ïƒ6X?헚s'?Î÷=Ô2?œQƒQ^´T?‹¶tTxÌ?¨]–@Œí?"À&—êO?ëßlà°?§èCBà­1? ·ˆ"œ?•ó¦Kr?¹øÔ²4Ç?¤`h§ô¥¦3FGL J2300.0+4053@YO‰ 'RTÀ1>%Øם
À:5D…kÀ;®ÖuÂú¼ÀøBÃIs@¹®@ð‹?ø9	Ü¿ïØfNq/Ì?îßë5v7¿ìÕ&sÃW?éV¸MäºTUNASNone?ïÍ{D0!±?zЃúy²?h2zT@}5?mÖS±BÖ5?jRA{ÑÃ?tÊØ«\?ïÍ"áú‰ï?{Wª5XV?PB;."_?WÝ2uŸ¹?u^75ÀS?x覰?íçøœOX?š"@buÑ4?ŸL‹["L?";wcîú?¡Ú8˜pä?^=w?`ÿ?ïúÈ'­bi?[R í[ã>ÐÎ.çˆÌ‰>óÝ©™ÿN?D½Äì§F¸?[£<炲3FGL J2300.1-3547@…Ø=CWnÀP66ŸÏ=ÀÀ:Iæ¯ÌâÀ;ðXr‡ÜÙ¿æ
zßwÓ@FEêE¾@z7?‡Ts?çh\eþÚ¿æpÙquä¿ãlŠ2¿â…f®'+`UNASNone?ïõËûM¾X?Xo»¶%#?%.®RuY8?)Íÿiv?QÂ3š4¥?V®¢»ÂQ,?ïÂΑÉi:?€ËÉ!ªl?LcÆÞ2Ï?[´Hÿ}ë?{Ê¢oœO?}À@§üÜ?î̊šÁ:Ï?‹aÔx7p?ˆÌ]]®?w0	D+?š}ùJ$X?…ƒZÎÂ:y?îÿÜ;Jѵ?—Ïv£3О?@"öï?CåP"b?Ÿ€Tõaá?—¢K^9äF3FGL J2303.7+5555@[
…Æ}þÀÃ@&`¼ÙÀ:@»â™½¬À;œÜD9õ?è»[.ò(@
Z[k5®?ü‰Ÿ¦xû¿Ü1튩ß?ïû­9ÙH¿×þ}êªr¿ä
4Ô?>UNASNone?î+Xžþ]m?±¿IXÛÑ÷?yLÆÔÃ:r?€Å;˜ùR?ª Ý5Áê?°²ÍÜw˜™?Ù¨åW¾ž?Ò´ÞÁ?Íßj_e'é?Æ]|Ø?Ø¡êõxo?Δ)îö³?í{ª‹?¢—v&'«?›Rí>9fþ?‹Aê/µR?°R Ø<Qî?ž"ŸnÕ$o?æJÕHs€G?¿gw¤_…%?Ðq÷ª¤‹´?¾ðۆ‰[?§Âî#£ð?¤dÒº­áž3FGL J2305.8+1658@Vqn?x»ÔÀC€¡UO¾À9Ø+{¯À;Aù¬ÿ§ë?҇‹-ŸÝ@´l8~L@3Œ¼¿éÌý°U®ï¿ì5 æO¿Úæ`æ¹vȿ纕KÅêõUNASNone?ïûËZTh?B	§øÞ|I?Ê'J+?üÑØ)Fê??5sÝ~©?A—-Ó³†Ò?ï&Å0&E?†4[ã¢Ëš?WÕ÷*´Ó?e>àÀQÓ?…»Îµ˜B?ƒâ–àˆý?îïø¡[§?$tf8\ì?ym¸ú¿F?ohjËÆ/?›Ä=•ÛU?ŒÝFêo{˜?ìð®J›åÉ?©'8'Ù®?XWBºÓ¢?[À.`?¸0 5ƒ-?©_öpôa3FGL J2309.0+5428@[}VlôÀÚüGä› À:Ž¯à,üÀ;¯§Í9WÀ:$¾ü*@<9·[ÌZ?û('¿/«>?ïÿ/FOÖ¾¿áî$gà±S¿ê+ÛjjN?Î_É4
UNASNone?42úß?Ÿ݉ðm?qågïK¾?^S–U«•?…`¾û›Æì?˜Šú]"Ÿ?î[¶`?ºÕÄ|™¼	?n.#øÈw?€LJ×?¨mŒE
r?¹æ™K¬î?í	(ú?Ÿ)¡­‡?£ N›y†"?"$˜uã?¬o€#óéÏ?•Tsý™ó²?ﺒð‰ò5?…(¶Q[6>æBPT?‹/»´	µ?U³9¯NÊ?…'¨‹Íþò3FGL J2313.1+3935@YÃxFÜ]À3uº² À9úò03¤rÀ;º7'´yð¿îñØ@I·yS~@Xk 7™¿éD©Qü¿êÀ›ñ¸"‡¿æPü¸*†ð¿Ô¢[oéUNASNone?ïïKP×Oƒ?béÐ{Ó~µ?C£(mGW??Lÿ òx´•?W—ʽM¨?]¸(½ƒ.?ïµúú Q?ƒÚC½£BB?Y4ñ(t4?dîɼ¤"?~½êF¥ºy?žòY<½?îý±'g?†ñaðh	â?¨¤ÔÒ3?r¾†è?—uš@³3×?ƒ-fÈ̦?ï¥qU»×?~¾Ö3C¦Þ?
—ÉìÙ?¹©CõQ?†{¥av9?~®QõY5í3FGL J2318.6-3829@vKÂã>ÿÀPáú~¶¿DÀ:Cê¡ô²À;úWâ?$Ù¿â"D‡»Ã@
Ò9u—‡@¡ß¹8›¿ã_'»Ëj¿áÑ)¨<l¿ásŠƒH–¿¿ïÿúw2šUNASNone?íÖl9ªû?¿\Åóºæ?–pj\×?® "xœÞ¥?§fÔ0$¡ð?·PM@ůå?î‰IPùjº?¨ç!㐕9?…î¯ÆÕ?©Ð†â"?¢ïjýb¬?£Ì9,»¶?êýûØ
¤?¥úCSOÏù?³HŒiؾÅ?œõ–wÑü(?´Ç"Õº!?Ÿ'Á±À¡†?í¡z#í?¢¢yžÊÊJ?ƒ0B]ÄD"?…~st,,_?°'ƒã(? ö÷ðäâ¥3FGL J2321.3+5113@[7ÙÓEŒÒÀ"Yò™0À:ƒ¯'R£;À;Åú¬(©¿òSdvL7'@
XÕȞê¼@&ˆ "ä¿âm
&õbB¿ç¡˜Á'l¿ÇÏÿc-f¿áÅÐÚ#UNASNone?ï1æd/­j?›U}ãU;±?@¯"å´^?E>.ô}0?™=·Rám?›"v;?îÜIÅuw6?§'º–Y~¾?löñoD?wÀLG? q"Féu¤?¥§§úE}Ì?îhOÿ9½ô?">·I\ú1?ˆ
¦ðf?u캧Ú@?£t<¢¼¤¶?'YjI‰?ï'ÙC†?¶M­"Ðå?
C؇/Ñ?"Sðñ?/kEô"?®RŸ!É#3FGL J2321.6-1619@KßÕÃÀP¤yèQÀ:Óe
 ÒsÀ;ÕSV¿)v¿;oX» …@
H€´ãw?ø†D 
é¿ïÿG+À^?ïÜèêi?à_ÝKRÂM¿âI:0¨iUNASNone?ïï²R•\²?q7J`ó?(›¶t?;jáς9?]—ç^"é?oÅÌvZŽä?ïŽ&`üÎú?–•àML=?fìmï"?D?Š·[n²Y?†»LDçqÈ?"²J)ÞJ?îÆáõt¦­?'¹M‹p_?fÔñ?ŠÉuêÙ?—¡E€±Ï?‡gboûã?ï˜Ú(ãñ?"K#Ü̺2?DzúóÍɉ?Yín4›?ˆ±ÙƊ'V?"
k`(R3FGL J2323.7+2523@XÇP%"õÀ@²õýG¾ÛÀ:{—)|ÑÀ;â%™È"¿å=äiÌwg@gGPvÿ@__¶ôÉ¿è?+~UgÞ¿Ü«'GËú¿Þ"ZT®ä¿â1@1ôDUNASNone?ïõÑ¢íµ?Q'5ßM?(ڝ4&Y&?(½$#uk9?QAgUŸÊ{?NÇP¿úÚ?ï¶_†=Gn?|ï«?¼^?QÉeƒ©z?Vpô¦!Q?€.ñÀ8õQ?zZ"½ä?ï9nñu«Ã?ƒ·Ryð?€9Ü(/¼`?q©•
œLØ?µ3½2©o?}Ìî+?™´?w¬"¤$YK?(£¬ v*Ð?*.C\sW?†®êæºH?wsàhɞÂ3FGL J2327.2-4130@uºü"µÜÆÀP㦠YŸÀ:LÚ")=À;¬sWæpã?Áa^68˜š@µîŒ:5†@4Ý ·0¿ä¬ÍlÍ¿äºà恡"¿ë1pΧËê¿àØ-ÚóoéUNASNone?ï|p¯š2?Ÿ³³:4?~Šh÷+}?"‹~æ¡W?•­×¬Aڈ?›H£á?îëÜ[k‡?ªQÑBšf?}öø¨ŽX?'¤†Adõ?›>vÔdùá?¤1Î7[*?í:À¦'Ñ1?ž'$A?œ3(±æKž?‰¸¯±‡¨G?®:aDÇ)?˜0¶ÞÅm?é>;ü?³ÜswœK"?˜žßjØW?—ùq.!?Çô=uÜ-?³ía‹53FGL J2329.8+6102@\M¶°_¯¿Òê~8•À9®ç¸5À;D
ð
­¿ç²9´¾@
:EÌ@|y ç¿è`ÎۚƿålMPjх¿ÇR!ïدH¿â¯3ŒUNASNone?î¨ZH–Ÿ™?§õb?^5
p"y¦?aõ2Øk›?¤ˆ³j¢?¦™#œiâ?µs"†›"€?ÄßífdÉZ?ž\ü\'#ý?©qëכ?ì^§ŒGüP?Æ?ÕpÔÀØ?ì¬þŽ•è²?¢'ŒÙáç?•Ä´Â4Z?"ÖIc\?µ&ÞZ×? ›a¥^øf?íǁú6ßÎ?£",.Œ?6¡gªº'?>mʵ>|'?±­îŒáVØ?£½â'íª3FGL J2331.9-1609@MÒR'ƒÓ_ÀQ$GÃ
0jÀ:5õáõSÀ;ç"6Æf?íEförý<@%Ƃýk@SÐ@Ô?éãÁ^¥…¿àK¯"dP¿Þ¥Y¨ŠD´¿ïôÃaû-ïUNASNone?îIž%Ž©?±·ð¦c2'?¦"æ
Mî?°AÁ
$PP?ƒDá
d~?"Ïà?é£:^áj^?Æ æà1«?¶ %ÞAw?ºgkæ?¼F*³–œ?º.³rE†?ç¼¼œÝ¨™?±ŒË
"ڇ?Å
¡sMš?¬,AvÕö€?·þ×ú, ?¤É|6ê›?çþWéûî?¾ñhܽ?¿Û¦½p?´¼¶Cqi?ÒwLùX??µFÔI2­3FGL J2333.0-5525@tC"Ðå`BÀM,k΅3±À9Ñï<c]À;ë›
ß½?í·&ÑaBK@
ð»äó	M@Åh`'6¿ÝèTZÓ¾·¿âïM,¿áéBËùày¿ïÿá_¥UNASNone?ßþlÆ
~4?ÉäuBñR'?ÉìŠl¡ÈJ?Âuöu¹'¯?ÓN¡¦?ÈUO´E¾ä?ÔS?ÞҎ;?Ì^fi-ÏK?܆ĪÐ
?ÊYâÕ³r?ÎKöìºÝt?Ä;ޟ¿?ãòS»¨?µh~°²ÙU?Ëç®ÜWh?°j‹i¶Õ?ÄO#Iù÷?¬>æö9]?ßlçV%˜?¾FÆHu.?Õmç#ìh?¿b~='¡;?ÇêcÜ?²ûžæõz3FGL J2334.4-7948@s1³g ù	ÀBX—{žÀ:OŽR=ºvÀ;ÃÍ¡Þâ?Çâ|_T¬Þ@ºý¡Uü@ø¨™Mn¿è›Ñ¯à'â¿ìitònƒ¿Ð½TÁMh¿æ
åH UUNASNone?ïêôsÏ?k0à¸*	\?Cø-ÆYz?Æ$'Ò?d9loŠ³n?jñKEº-?î¨TÃÇ û?«j´X3r?€Ê}qPÐ?,9®++?¡Hg9ì ?¦Á±¯Ï>?î"R¯Œx?"öTI^Ó?‹q>&óŠô?x"xa±vM?¦þ…}{›Ó?'Æ!`ÿ?ìIxãõ¦Á?¬7Ò	"͜?ysŽǬµ?€—R¸œ]?¼ü·fO/?«–ƒÚiãŽ3FGL J2335.6-2342@DW´ÀR#¶þ.n¨À:PJ›.ÅÀ;Ø*>—ëD¿ñ#†TÃPÍ@×8Ëùh6@-à_PÈ¿åÍ¹¿èy1ÈÇ¿éwíÒ"nŒ¿ß#<*R¹áUNASNone?ï£V¿¥ÎF?¡Kƒ±'–?kš½‰Ç†?'£¬…>î?€C ²©ü°?šÅ '"?ï$xDTv?°«½#žÂÞ?òJ¢À?ˆ0é×I–?—wglç.?­ÏçwµØ?í›wÙÑd·?˜ñùÕAÞí?–¼`4F?…fÒ ­
?ªêz2ßu?"N°+¦ò4?í˜D*EÞ'?§`ÒMÞ¦?ZFÜçÍdN?b
©çD>X?²ÔÃ:1Ù8?§@»Er 3FGL J2337.2-8425@s}ŠüÀ@3EbàŸèÀ:v"Z»7À;¬1u¿¾ÚS"´,@
C˜LgŒ¬@ ­`uᄿÔΣUt¿æ;º{ïî¿èì|•å…?ÏwžëUNASNone?ï±gHðgc?…L²eØG?`ÑÀ›º‰?h|ƒ:è8?~ãyÇ~q7?ƒªokp?ï_×}|L?£¤0d …³?p+×?þ©M?‹­BÀ Æl?ô5á˜q?Jþ•à¾?팪cœ¥ì?šö6¥aùw? Sðí–<?'Ûd'ÊUó?¦ái¿H
?'ÛeÈ?íï¨R\?¨¢
â'
Â?`zvÂ(?r¹M¼–*?°ú;Y·?¨}¾šV\:3FGL J2337.5+4108@[ÓØYÈÉÀ3ž¢	ª£­À:eÉÞÜÀ;Д9ˆŠ?Å+á×¢@@&Ít<"@ÎçßwÊ<¿Ý!.üö=è¿ìÈöÑ$—±?ÙJ»	ÖÃq¿í–©C'ŒUNASNone?ºç?§1ãeI?Ñ	¢Øþ¶?‰í—NI—?¡C|+›Nü?¤\÷± ›?íØzv®¯?»•3#*ñj?¢u¶É‡ëò?¯'±ÎÅUÞ?«¬Á
)?°åI6Ý?êâr!ô°?¨ÛšÚì?³Ìqm´´ù? M¤?XL?µý'«…? rE
Ù?ìÉÔÀN{?µ%26ø?réù,E?ˆ¹´·E¦ô?¸'ɯ̉e?´šÜòÁõ´3FGL J2338.7+0251@VsI''>ÀK¢±Ä2ÊXÀ:)>ku™àÀ;Çöåv?â#Œò
Æ_@ÛNšÂ¹y@¡u`F²¿ãÜ©""#2¿çuiÛa²¿êÿw(«¿î.'7$¯UNASNone?ï9Š]××?§Úd¼2W?'©úI©?
ôüáÿ?ƒÓ-ùÀ—?+©r…?î7ͳ<	o?§7øò«Ì??ü'ï·?˜zRåéÏ?¥3%Ì­/?¢Qö=Ž½7?í"Ð[x¿ç?œ(>Ú/½?¢ÇçBª!?Èâ"÷‡'?£ûcWb?'=†&K?遀ñyÍ?®ŒNr¤þ$?²F€3Ÿ? ‡Z¶Ê©È?ÀùÜd IN?©óN¤š|3FGL J2340.7+3847@[	H˒:À6	zû]À:Ž§©&ÕWÀ;Ô¡¹"ËÝ?°áȚS¡ê@
µp%¬âÍ?þ³ŽÀL¶½¿ë>¿0,¶¿í‡¶	U®?ÞXä¾í!g¿ÜB"Š;,ÒUNASNone?ïî‡åLÍx?`éšÉ/ú?KQIœ¼? l%ns?`¥Â˜¨;?`¥eAƒ.?ï©´vésJ?‰
¶ÄLs£?[•ÝÏí¡ì?b"Eš½h?' &‹¥y5?‡2¢@'?îä¤_?Š–³ð6Ðæ?{ð–z!áy?i²rDÝ?œoN}¥"?ˆv;óe?ïc²	ž?"³©J¢æ(?:fzŽ?1~B°!–:?"s"a-Â?"¯gUÁZ3FGL J2343.0-4748@t³Ý)4­ÀPY6z—À9áB-¡úÀ;Ü÷'þL?äzZ3I¥Þ@
%}$p@HVßà¥È¿×°֜•‰¿á$ÂÛ:Š¿ãDvcMq¿æç×FÅ®˜UNASNone@?ì(jÈßF²?¸öݑí?ŠJú?Œí!?Žø½)¢ã?»sJq,Ã?·XÙtݒ?ëÀˆi2N?¼"#ŠÍ Ÿ?¦g‹Î\Q?¨ÉÓýÒIâ?¶Ç÷6¿?j?´á³Þ€_%?ì«*%•þî?£–µï¦h?¤(Ÿº> ?'ú
‹žr?°'¦réƒ?›>‹'þ9	?çÜÁ–¹;?²<ǬVí?³å‹ã‡¹?¤®Ëµ°Å?ƜÛ2³W5?¯ºr×nÌ3FGL J2344.9-5647@t¶®}VmÀM/]»œúÀ:éÊ3•YÀ;÷ÂÅ+?Ç<;±'@W½þ¨¼ø@'3ÀvÓ¿â·Î?ŠüÀ¿êOüÁ¥8¿é'Þ¸©÷'¿ïÿååè=UNASNone?ïñ0ÙbJÃ?'Àó]ÎÛ?/Þu‡òeP?MOñ ~?Y¢~Šl/9?'¸©Íd*?ïÈ+ŽÏð?†ã{ýž?z8@…,?'"ö¢ùÒz?™Xê†D·?˜h["ýŽ?îq'³'ß‹?'QXë¾'?•`;ØÊe?"g'Qov½?œmm´Ù©'?‹ðЛŒŠ?í8Ô¬+Õ?¦¯B÷pÀ?•ÇcüÇé?%r÷h/Z?°õ¨Â÷oc?¤G­ÆP_Ï3FGL J2351.9-7601@s9ÈýŸÓoÀDFÂß
A1À:N2 ä|À;­.ƒ¡	пۗA¹øx'@š÷0£‹á?û›A9†4¿ïÿ⿹z?ïþÌì­<å¿Ñ	Bsíã¿ÜS.¡UNASNone?ïúAV£š?O¦ ÆÈÆ+?‹€Æú¢
?Õêãuó?D	5Zî?p?N'ìW‡bÜ?ï}8VôŽÇ?"ƒÿôI×g?d–í{n•V?Ñî8WD•?‹Œ.ä¨ü?,£e%vŒ?ï	èË+U?‡ÔMž÷?€GÂC[ô½?pX‰øɚ)?–ŸxçcË?…
"ÉN©?ïY/]E»'?"³ÍNˆ?k>œá9‹?oòœ¯DŒá?'r@»!\b?'þirx(O3FGL J2354.0+2722@Zär\=îxÀ@ãÈ}²³FÀ:«ks¡RÀ;þ¢$'–H?Á{µÚv@
œ&"iY
@=ÿg©²¿ìs_ôx¿ÔŠÜŽG׿ǭ€'ú•¿é°6¿UNASNone?Z'_ì? ºgÊÆÇG?r´žed€? D…iª´?}ˆCj¥V?~ŒóƒsÐ?ï$<­z—?•êB¡Ýc?tEƒè¦æF?x=\Ž®¾+?–g	V"3œ?'})u?íÔáü4R?žȱÀc?? 04ƒNð¦?•_$V¥þ?¢«¹pJ-?o·háP?îûC­Oxb?"ÈÆÜy?È?np=©,?pm$íRËÖ?œÉ‡®[Òö?'2`ûÒ3FGL J2354.4-6612@s}¼¾aÐÀH÷'·þ	À:?ïXzÀ<»Üº€š?؆èrÖÈ_@"Ú§
@€å¿ŒóC¿àSžˆÛ¿âæoÇIfb¿èGÇûèÕ¿æ†P´@~UNASNone?íȕÄ{?±Ç.F %ù?žú¸ ])?¨ÑÁ_ìöa?©&+'mÙÌ?§£ÿ¬Ï^?íØíˆ	š?°ü{"/?—˜¯Ë?•ùÖÉo/?«A~·ã?«ùœYÇ??ìÄ%éùµC?¡úáÜ°*R?¤:[P´¾°?"ê%Wmø|?¯ƒF¯í/?—˜Üh'G?ì&ö|¬?¨À©)T|ó?¢ÔaÍá?–|à !?µdÿe
œ?¥^ÆÆd¥p3FGL J2354.8-5245@tº^5?}ÀO#ˆDÀÀ:åw¾}À;¡7qÁ
?ó!–é$e@q"T[!@C}ßÔ¼Z¿è¯S´KæL¿áòUÎÈ¿æQێþØZ¿ïÿóì)$UNASNone?åÛìyÐö?Ì7ü¼Ã'c?βH€¨úH?ȗéQ_D?³¼*߃Ç?ºìl(`?駭—~Õ?ÂU‹#ßtù?µæMsŠ®?´¹üüÆ}\?¼ÜŒúp~©?·u'œÁjÝ?àˆ›8'?·xA²ü3î?Õg£•"ø¶?´ï¯aMŽ?ÃLË÷ L?ª³,þé}?âuüµÈ¼d?¹0ƒLÖ!6?ÌÖ÷tœ°¶?¸8 Ö§85?ÉQ´@]¸?°¹øuÐTª3FGL J2355.4+6939@]"_®¼@Ž@<œaÊö3À9±a8)<9À;)L$›À»?Ëý5U@
Ò	ÿ2O³@[á ŽÂ?Å%£'·Ôî¿éÞm^°Ã
¿ëšMbx4¿ØôMyÁžUNASNone?êK'ú	J?ÃåϐÕjÐ?¡c}5j?¥œô¾ïÕÙ?Âzª¦½Tô?¸€OÆz?ì i²þS1?¾‡
nG?Š¢ÕÇ(#?–{¹ʪØ?»¨W¯(b?»ÎlÛ,àÓ?èïrCŒ]š?²5îcÝM?¯!ã|'½w?š•o"óœ!?Äy¾ª7?°EÚ_ýG¡?è±YV.%?µð±•¡aã?"_\4mc'?•&B¤ü:?Êί ¹¿"?µŠj–sÛÑ3FGL J2356.9+6812@]yèPð@'ó!Ë+ãÀ9oÑI3PÀ:ÌÀˆì?ӍŠÛCe¹@âŒQ²z;@
Aߞ`©¿ç÷݆S¿ëš{8Qøh¿çì"2Á¿ä:Ä—UNASNone?åTÊ*ZÍ&?Éñ¶Ežú§?ê ü+?'}1Sã€?ÔVK¨Uó?ÉÚ5~Ÿ1é?ê_vŒÅÜ?Ã3¢¾ÛöÛ?'"[ŽÂ?—†0NÂD?Ä1b³úðA?ÁÈ-©u]?áË6׺#?¹§!'Q¢~?¶üdÂ@f?¢YÜc"K?ÖªØaÀr8?¸&âYëy?⧸Eu®Ü?¹˜Å=˦—?–fހ{S?aEÿ²a?ÙJ!í?¹-÷cÇ؋3FGL J2358.5+3827@[ëúÁҝÇÀ7BŒG¡AÀ:0/(âwYÀ;¹‰Úõr¿ØŠ$¾@¨ZéZ¢
@Ÿ?Àà?ïӇ¶–¿âØem~¿â"'«ìW'¿ØÐÁ'°ÁUNASNone?ïõŽWÝ3ß?M#'Çñ?.Në|‰
?+AÁ"dsí?Qr∯ý?J˜!ǦÔl?ï³Ç»ú`?"©ƒf´<ü?XC>æ^Õ?]³Cµú6Þ?€4f4A;ö?'ï´ÜfN?îûxjи‰?†ˆÁ
¥pÈ?‡lpIeö¾?vú‰ƒP2?"Úº5ó‰?€["ú»sf?ïÓ3õ3U?•h§%îØó?FnŒã‹HÐ?J%ãi§Ñ1?žr%=;(?•5¸ûiq÷3FGL J2358.6-1809@P¦ ºKÀR¹G"#ÐÀ:SãD8>À;Äꁺ?今ã¦á‰@.ÉA'?ý`ç÷K¿è£p™+pØ¿š¸þ{Õë-¿ÉÁ2\@:¿ââôxQ9GUNASNone?ïé/B?vXq‰»z?8Õ÷ô–È?BÀÎlÒªÈ?cÑ@Ò:÷¸?u~6b?ï]þd¨"ß?—2T¤Ã-?d
1T9?jî‹<?'¾GƒQ?•Ö¸3˜þ>?ï,¿¬èT?ŠÏþ½¦O?'¹'¨¤î³?t´¶~Ã<è?"½Ÿ6~1?…gp~O‰?î^|Åâ²Ê?ŸšÚ>ÑQ?pü0¥F˜?sú½ëiH?§ø­,q?žÛ\Oö63FGL J0002.6+6218@]SRÁmóù¿£äVAÀ8¸4t{ÒßÀ;¿"å­?ÿ®	&šI@ù8ö–Ÿ¿?÷;Q­Fʕ¿Áôˎ´8V¿àõø8Ðø¿çϟA›£,¿ïÿÐ%­õ­UNASNone?tiHëÿÌ&?{ãñùÒ
€?ç(Òñßz ?Ì€…ZX?Ñ\´ø''?Ì:Õ²a?ÉpÀ2?>'¦ÚÚÏJ?à¹zZ[¦å?φ©ZM#¦?ދ޴<°u?χ‡… n¦?œògÙ?¥ðvêP¬?ê¹™•š9?­X»uÇم?Áˆ!;iŠ?ª­ˆ#ñú1?"Þú Ø?"Ðì64ú?쎏‰µ?­š×&0?º«ÍOÊ?«mƒÀŒ1î3FGL J0008.5+6853@]ÄOÊB®Ñ@Y»j¤¹ˆÀ9u(>«	À;e£Z»Ð?ýí,€çq@s[T9"?÷ðΑÈêÀ¿Äæ}ß+¿äY_쓀j¿î¾£Fõ¿ïÿbá*¼UNASNone?'ª°{@²·?™G•œ$?çVthô?Îÿð%}î×?Ð8l(ôí?Î~a÷ˆ‡š?n6ߪ‰?œòÙ£?è€vk€GÎ?ɱ&®µÑt?ͅJÓT¼p?ÉXRýdnà?¼a
¥<´,?¦»'à—?çAÙÍK÷?±"ÚüÏè?ÄÈx1Éj?«*º8?‹ë>?"<þɊܶ?íµ/Þî"?­U
å*??­åÔÁ	Q¾?ªÑ×ÇeõÜ3FGL J0008.7+6558@]¦s>»ýr@¤á¼©iÀ9šCã…À;,rÉK8?ý—£FÉ@ÏzÒB@pp€p¨µ¿Ù»0(wÿ¿ëÈvaŽÃÛ¿ãôÄN4Q§¿é쌦t¦úUNASNone?¬ÀMÛ'ñ#?ª.¡¢¡Ä?ØNŽ#Ò?͵>"(Ä?â´ ;ü…?Î9íã°ü?¨ +|T›?²ÃC Ý´d?Ù.̸ŠV?Ë<3¤™Èl?áޖëú²?ËP "LTì?ÕìžÒN´Ò?±O£6?؇Ê8Q•Ž?³à¬DE٘?ы–õ_µ ?¯£Û–¿?ú?ÁÓ(G]Ù?²,¿áò?áۘR?Ç!¥•ÂA?Ó_;²?ºq?Áyœ´f3FGL J0039.3+6256@^c {5*"?º$ª.gF‹À9köÔ{À;AŠ[@	.êú	q@;epÈ¿Á'áÙ¬âª?ïý°3Rׂ?yѦ p&ô¿áä³Ä›®¿ïÿü]šK,UNASNone?ÌñpcàÁ?Ӗš …x?æxÏ"Ö ‰?Ô±+[§‹?²Wd€‡:/?Ã%ã'o?w–
$"†œ?¦;å>Ýï?ÝzÇ=Î3?ÔM¼ ²B}?ápM*oÙ?ÔPX3qר?´ ë-r?¤S‹O4a"?é1üîèœê?°Fˆ
\9?À疾Gœ?¬RãÌ*Á?¶%M1,c?³Îýy0Wu?éŽ,éÖs?ÃWn9êUi?½iK€38?¾²Ø僌3FGL J0212.1+5320@`ݧæšÔÀ•&Rz XÀ8ÊYž×ÇÀ;/`Ëò¥?ýyšóṙ@‡/Kòò¦?öۘð&n)?Lóp*¿Ùë»{–¤¿å¤þLf`¿í—*;:ØUNASNone?s$<¦»<?t¿ÄïÂÊ?í4ȑ'W7?½ÕDp(ý8?µ'yïªÚ?½Hê=† ?‰þÔHÇÒ_?¢›¹‡ï½?é~ÌB¤?Äs&S/Ձ?ÊHÀBxN?ý0"Ÿ¼K?œ§,ŽÑ?ŽQiÄQª(?ëP™>²W?¨à˜÷6E?¾Qp'"#á?¦^èIçó?©ÌB;®?–ÊP‰…ïN?éÜIeꔱ?²£œVSz?ÂÖ…Q?°… ñ'3FGL J0223.6+6204@`¯âXOLn?ñצ_z¹ÛÀ7ò˜ëô°AÀ9àá"-nÎ@»Ð¸ê—¹@
ۚ?±Æ·?ùŽùÕÄm-¿ãÿī웿ہU§Éª{¿ç䌳w¸¿ïÿÖܽ}UNASNone?@	H¶C@ ?B…1ؾ	A?áÅ+ÖÝáÖ?ÐÐðÂ3®w?Üm£­é´?ÐѕǺGß?WÀn¯|¼?pjm³4Rì?覀êîÜJ?ŧZI¨?Í6{væuâ?ŪƒV]¯t?šWpÚó˜?'w¡ªÇŒ;?å[T"ä¿?·ž»ÐdSì?Ó¤bJ
üø?·Gh™VžÛ?q²É'¢Ä?q¾^õ3FV?å]~w!i€?ÃAWgî?Ôþ7ëuw?ÃX²Sõbv3FGL J0225.8+6159@`¸åŸ+©Ò?ñîI9.õ·À8\'jPÀ:ç!éB?úÁ.ãÃ3@¿v×LØv?ü9´¡ÝµÓ?ﻼG¬š¿å"à…Cÿ½¿éäñ
¼¿ï|w@9'.UNASNone?UÂç჎?]žUEÖ-?Å?t¹'?Æõ'°÷Æ(?ê´®çÏð?Çâœ~.%?kî:yàí‰?'mnMg—ä?ßþýEz.Ã?ÌìÙÌ°ý¥?ßÉ&E'b?͵^?¢T^Tü?"^áû!½¸?ØùA&€ˆs?¸»+[P@Õ?â^‡oñø?¹!åZb/¡?‰6E#oj?"ô2솈?Þ¯Aћãè?ı¯_Y"ˆ?àC†¶€N?ÄÃpª$=å3FGL J0238.0+5237@a[&ÉÀ¯"á¬WâÀ9.ŸÇ±À;pÌ؋Fð?ø4eø­P[@ËÊÒ÷‰9?ý;3L³Œà¿âo5ãå¿àà¼;bµ5¿ä&â涿ïÿéò§}UNASNone?¢ÎlÞNÑ?¤Ä9/›î?᳋•ª?ÐK—
Ýõ?Ú@-<A
Ó?Ð|Â\/?gìÂìÀGð?vI•e«¶?éq|Žp	é?Â×;䮦Ü?ÉÚZºŒ×=?ÂÂuÎ5?Å)HíI ü?ªîþT(?åLÄgÝ?³
øaJ?Å£¦Á?Œ?ªŸ€ØÛK?°žÝ9·,ü?ž¦FÉÞ?êëCm¡Ê?²'öÅÁ©?¾ÑȪÛÄ´?«ÌÇÓÇø3FGL J0312.1-0921@gðwÙUqLÀJ.U⊤3À9ùíÓ­'žÀ;ͤ¦©M?ö2´ [)Ç@åYŒä)‹?ñ7ð<ªÒ?ÚDñ«±þ¿ßb{$¹rÓ¿â±ï¿¿ïÿö‰£q#UNASNone?Ùý=äŽÒz?ÑÓ"?× ÷ËW?ÒuTêØ?ÍĂòÄ`?Ííöý߅K?ÌN®Þ¹	A?ËA¾A–¸œ?á'Öaã)?ÏÅg5O?ÏÙÇ¿j?Ä·'g?ÌUC9èð?²ä3J»™
?ã÷§ø¿°?¸*Ôݸ%?ÇZ ãM?±@jóõ¥?ÕÈè1ã?¾øãÍõ©Ô?ÚÖür ˜¤?ÂÙ³A‹å?ÎÀ6·ø·œ?Àhuú´é3FGL J0318.1+0252@fN>ê šªÀEÑG®záÀ9ãpñãºÀ;îu"çZî?ûô`΢:@TÍ¿»í,?Ñc"šë¿Ï¡CS‰6l¿½F$ð'è¿åðÄ4,¿îz]ûͅUNASNone?—¥M^@¹œ?°¿¤SÀ?ìS‹ÙjœI?Å®|?þÅ7?·zMÝïQ?ÂÝMV9uù?»É‹œå]?ÃïUÈ×"Ð?ä™f³E†E?ÐK4K"Zè?ϵÝít>?ÈjêaRN?²Ãaëóá ?¢›–
yê;?ém\Á×?±ªàMñI,?ÀèÞÇ£Õ?«(·blâ?Ϫ©ÐÑý?Âbaòa§?ãù¶Qï½?Æï‹è/½?Àý|p9Ñ?¿NmINª3FGL J0332.4+6110@a¤u£KÜ@'h	ԕÀ9¥¦&oÖRÀ;]Æ!·à¬?ö£câ"@Ñ•aüt@>í8}¿Ñ½±•¨¿ê?ùái"?¿ê"oGØÔ¿ïÿ3HE­ÎUNASNone?ÖÃhÇÃ]ô?ÇlÁVµ6Y?Óý¢³½î‹?ÇË)P°à?Õ>ô"~³'?Éwm§+é?»Êc¢pqÉ?ÁĞ>Ž#k?Ýþ¾dJ3î?Ë;N%Y_?Û¨³¯¡?˔×&ë|??ÖÎjÔ¸º?²^¥'Ð]?ÛL\˜ˆÁÉ?²V'6T–y?ËË)ùE
û?®èSÉ=Ò?Ï6Ü"?¯Y»SÊ<?äpf^?À—9Ó-9?ËóâMó?¸Î'Uð¿3FGL J0336.1+7500@`£~=Á@/¼˜¢"ÕÀ9TîDì™À;—éŠrµ?øÀaÖá@,Ó¯*.?øûiÁƒ¿ÓiՒZ9¿Ü0®.ã(•¿ä׆‰ÇiŒ¿ë)'Jê‡UNASNone?ŠfTC -P?‹mi¯ö"å?í€Œ%?º4Ñ#ÓÉ?°²Ñ"‰-?¹pé*D4?›$WNiÝ?­—'|C³c?쇥@en?¼Àô£ëêŠ?´ùÓx):?·(•Ç¶?º½Q¼h?«ÕUñyL?éõz8Z?²¡F`ì´?¼'ÅqÕ?¥™È
W?±G¦Lã8ƒ?žúob·Ñ?ë3†‡¥‹?­tÁ'iL7?µµ~ߛ!?¦`Gvƒqä3FGL J0340.4+5302@bXüø
Ã7¿ýí©¼&ŒÀ8ðà9'À;¸h'¹Ñ?üˆY«ìØ@»OÞ9±¨@ÚYO§ˆ¿åÀï7Ë¿îx¿ž)æ¿ïÿ}…^F¿á@ùðÏéëUNASNone?Ô,´µ9p˜?ÍÑQÔ®C?ݶ"×Mæž?Ð×Z‡[‰?Ì9ŒæñQ˜?É«>«C­n?˜'ë3éZ?²¯ñ%
m?àey6ê±}?ÐïÄYiCÕ?ݬÞÞú.q?ЗR©š'?Û\¨RÀÆ?²žýA˜LA?Òm•X@Ù?±›Eþ$?Ò5Â(l½`?±M–[NÕ?±Ú@›àϑ?²ÿ+Ã
Ô?潝-—º?Îë%Í ðY?οé=Y9L?Éï8
8í3FGL J0345.3+3236@d
ʁ˜ñÔÀ1ZbwÄ\¼À9‡G.'º'À;†@@aïß?ùÄ9-D‰@øc^J8?þÑe*|*s¿¸'©öB¨¿éQDɼ*¿êÛåIxøm¿Üš¾ZԍUNASNone?êë­Psæ?ÀQ{¸¡"p?½" ãý×o?½eXMÑx?¦é0ÓÂÃ?¨¨˜"ÊÊ?ëÄ×ǤÑ$?ij%‹›O?¬ìÚiR'?·
{Ê[=e?³bԎ0.?¸}»f¬J}?â—8y°ç×?µìmñäç?ϒzY?±òB¡‹Â]?Ƥ6^J?°0sëðM?âÏØ0…?ÂíÙyüR?ƞ0á>?ÃñËtøÄë?Î"n^Ô¦?¿‹4£`"3FGL J0359.5+5413@bˆLYtæ\?ëæðY|sÀ8nÌ¡-â'À:÷c°©€—?ý3ù;듌@Ÿô§‡C?ük—›<±â¿Öa78·"¿âi‰Ë45+¿æ7ÛÓ>Æ¿ïÿç—åu¡UNASNone?h›Ù"Òß?rG/QÄø\?äp´H¾ª?Ð\ùm'ú?Öí_¼{¢T?Ð\Üì‡5o?+m͇µFÜ?HêIÞL_W?èÂÿÃJ?Èߍ–'X?Ì𴍑µŠ?ÈÝþIƒw?©³Mêüj?˜³hÞv:i?èz'mœÇÁ?°²7­Vô9?ÇÒ5v!á?®5(¿œä'?w>³Ü
î˜?p‡-­<Ò¾?í
^d	{8?©¹gWQT'?¶!!¡óGO?¨Â…êk3FGL J0426.7+5437@bÛ¾ ºK@ý¸ýâïNÀ8'£A¹ôÀ:¤UÖÌ*@PŠÇn¾ú@•†ø,L?ýæðõvO¿ÌÖùͶ¿ãUº¿ìÝõ›W_¿ïÿDUNASNone?–™w˜Öza?œ/{'v?ênG/t»É?Å¢—%Çv?Ãs´OA?ĸ|µð²?}ÐYŒ?‹"($´éY?䖪Aí<M?ÊÂ÷pi¸H?Ö^Oä!7?ʲ¨I¸¬Ÿ?¤}¸i?•Ô!¬ÅxÙ?çMê3Pö?µa|‰"?ÍÆ·Ä¡À?´·¿­Y8?'WèýÐ'D?†'X*œ?êN~ž?{?¶‡™Úƒí#?ěáÌý/?µ#Ž'RŸ3FGL J0431.7+3503@d·BZîc À!Ûà›¶ªLÀ9Aû§««À;"n@O{?ö>?Þ½:3@cŸa¯@¿ó£%^‰¿æcb	¬Éo¿éIjX×v¿ãH VÑaÌ¿ïÿÃλ(NUNASNone?Úýê–?2?ʋó 5Y?ǜ;Ô¶8ž?Ã#™ùgg?Ù3÷e±œ?ËòD'¤?Àó‹f}ø?Á
{¬[ØE?Þ8`F
ç‹?Æ Ô!Ã?ÙMÚ+¾Ùy?Å焼«C?ܕHn¦y7?³e¨Ý,?Ö=@!ŒðN?°åiï¥÷~?ÊZîߙ,ù?¬$ß¡å?ÍküZ8ƒ?³*0
5l?ؘ£ì??ÀSMz˜ù?زcÝæÈ~?¹b Î<03FGL J0514.6-4406@o/-w1ÅÀA²DêÀ:å	ÚtUÀ;Õâ˜,ž?öýOòÁ`@K&Ðú.@œ¹a`B¿Øda~u%ò¿æñye­¿ý¿ïÿäÙ«Nð?ïÅ7ƒ5:[UNASNone?î(Ö£Ô;X?²'™¢ÁÎA?¥ó7Ö¹5?°¿ñ(?ýw°ù.?"IµÏ¬Hu?Ú*"Ú? Neeù?d›côhZH?†—í·˜?‰sðxD²ê?˜d¶IãÐÝ?ç½°óÙä;?±odXy¶?Äx¼Ó?­…o4*øú?¹!5ŠÄé?¢Ü&\@øÖ?ïf3Ü÷ðU?ž›ˆ½<i?lÀ*TvâÓ?Ž
ù4«í?Bþ,æ2?™ZNíӐ3FGL J0537.0+0957@hiŠ	ÞÀ'(÷À9˜K»ÀÀ;2(@éÈ?÷¸ß9áÎ@ÒåE°a@M:*ž9<¿àNéÐÒk¿ên¹ª¿ì\kñô,@¿ïï–û¦÷HUNASNone?ïº->øh†?Lö˜0?hsLقðÇ?jˆªbvð?v¯º
DÃ?…Rfhî?îSGtí¥±?²ÐÆ}‡Ò?†+q°h?"=vÝà·ñ?¥@ôøÕ?®À"û<Ö?ì†JñV'¨?¥šÆ¯ÚÐ]?°!aÐ1?ž"Óö©X-?§XJƒ?™Ž-F-7E?ì–inÑ?¯ÊUԙä? £ÂŽX?¡x@ÿª6ü?²úì¨0—?©Ç±šYõ3FGL J0539.2-0536@j5®h]·kÀ2›bÇut÷À9@[9âyÝÀ;3whí)d?úAN*…@WMç'@oñ§ÍŽê¿ÄеuÔS»¿ìÝÔ'¿çžr'—ír¿ì'äuNÐaUNASNone?¢&K1ƒ€é?¥Hš%‰d‰?éS§AÏÁ?È	5ÆT¾·?Å–—àÃ?ÅŹ1EÇ?¨¹"¥.ÎÅ?µH•Ç:»?ê+ä½soq?ÃmõÖ>ÑÍ?Á" 掐?ºÛ6q NÞ?Òêå6roï?±&`¢ßÑ?ߘ´r¶o?²x4.?ái?ÊøÍr5³F?«0¬Þè5\?¡F¨'О?•XèšÉ?ç	Ѭ^?Á"WŽ[ÔH?ϕ/-ÓÇ?Àè+m^3FGL J0541.1+3553@e²PÅë1<@¼÷S½À8¹ÈÓC"À:É(çÖz?üӮɺe@{%Y*éŽ?þáñ¿Ò̒…(Ht¿äh³Î¶W¿é¦Îb›x
¿ïÿÃÖȽãUNASNone?‹©E¤KÖL?÷þnxpÖ?ãK³"¤ïð?Юª"«¦W?؋O"Áo?ИóS†È?_Óü$š*È?t<[—¡¾Ò?ê"Òtr?Á¦³óZ?Ç5•ä•ç?Á˜ñ}g?°F'õф?œ3;+³qÖ?åví«£«?¶/ˆÏ
¢?ÑÎ?ëDJ?´ÿrùf?€P÷)½WÙ?uÿ¥ôP'?ëZ!"aã?²cE•L´?Á'j<þ¢ô?±…¸s'í3FGL J0545.6+6019@câXOLn@/©Á/	ÙÀ9'jËΠÀ;®.Me?øKÂ@¨^ùŠšù?ïdã&€rV?ۇŒ»ÿd¿ÓÂÊ$ú¿ÙWÍW\¿éƒ'ÆSÈUNASNone?ÁÉ»¦AÆ?¿¼Þ_¥Ç?ç&s"gN?ÉÌÉrø›?ÂPh3ø!?Äm¼Ûy,Q?§|ZÃ×\?°m¾ø/&?ê¾fö¬é?ÁoÈ(Di¸?¾NÁ!¸­?¾åºóôÄ?ÔG±(R?¹‰I¯Ì?ásø^*¾?»Ÿ	ˆc½I?Á2ÍÎp°ü?ªáÅD
Ï?˂8"?·~³gA<?ä3!†
è?À!iž(«]?ñj¯²U?µÍ"卩¬3FGL J0634.1+0424@iáXâe¿ýRøBÀ7Ȗ'•¿À:'zÁg>@Î郑Åe@¿Ê˜@"—hk¿ÓÎÿ‰"ðâ¿è"Dtñf¿ë0yTª§3¿ël›ÿÐZKUNASNone?}s܅ßs¢?"ž
‡êóï?å'Ì'¹ûË?ÏdGö…cI?Ôd—htŠœ?Ïu`r?$!ÓDÊÝ?EÆQ'^áª?굉©¶?Â~j*T1s?Çà¥d‡õ?Â|êó³‹È?±6‰+? Ô~Å¿û¿?ßëi –X?¸œ÷ù°?ÛÇNL#æ?¹è Ø3ŽÍ?sG]Ùl$î?p)ªÃ®Ú?ëœd±ðß?³8§y.´n?ÀõG~lÛ\?²¼e¹®
Ö3FGL J0637.5+0418@ið9–ú'è¿ñßX{ÆJÀ8ÅÞSÝͦÀ:¼hA1ùw?ú¶dÙ"@@p"Í@zlnh¿Âۃ«¾οêCnJœ—Œ¿èÌ׫ðV¿ëÚõªµ/UNASNone?Óù3i'±?È)ôв®?Ãßéj"?†¯×qŸŸ?á>îEðšƒ?ÌðìöÓ?•à`‡ãvÆ?¤ôáEUÁõ?ʱÝå3Þ´?žŸæ??褅'sì?Æ!'¹é=F?Ñã}º\?µ©eÃDé"?ÑçøÒîÇJ?²6û¿'OÏ?Ü4‰sܜ?¸—Õ!' f?ёiÅqď?¶Fæ¨w6&?Í7ÔÊæ§?½$Åöè ?ßÒ¬:(È?¼ï(:oÊ=3FGL J0641.1+1004@iY;%oü@õ¡lèÀ8·àªÐ"ÃÀ:¾­'tâ*?øz0gQ@†IŸ0\i@ªñó—¿âE":{•¼¿çOx1P@E¿ï¹8Î?Ð W3¯tUNASNone?×áûô¾L?ÓÏ}JŒ7"?иҪV^á?̶"wíÓå?×f Y´âÓ?Ñ
Ä>å¡?⫸ý²X?ÕÑ'nJèÓ?¥£DzAË?³Å¬q>ï;?×ô*<¤?ÔoTªJ?×EtÎ'""?¶c¬tº?ʵ
ׯ®w?­'ySÕ9?Û`Ƥ1?¶¨PJ€Ð!?áp¹YêÈ?ʔšß'?¹Z2Sš­?ÅNçQF:ˆ?׈˜À·CÅ?É9bbœ3FGL J0704.1-1043@kýHýŸÓoÀ¯"¼
êÀ8ƲœŸÞWÀ:W™?÷Omü]@
µEw•Ü@@-Ëë%¿á¨|&Ö¿èû0•ý‹d¿æì.wпëAßQsUNASNone?ƒÏÅÖAÞÝ?ƒe_\ÎXk?ɶ™ÏË?ƣٔ
ê,?émÓB3Ã?ÆåUžÕ¿?‰½"¨«Ã3?›ñ™ˆ°Q?àÃ~'Ïeo?Êè$՗D'?Ý«‹×?ÊÉôä™$Ð?Èüڑñ
ñ?®/ä.ºß?ÕxSùœ3?³"#¤†ó?Þ	>½jÛÓ?¶A¤Ù@?¶³X^mÁ?¤K'ú¥Å?Ùîr€Ä…?¿F˜œd»?à2f'ï¹?½B×4š r3FGL J0711.1-1037@làuöý"¿à"5Iè‹À8õLÓi©À:˼zo1ç?ø—h\4ß0@
?Qkr•@¼1ÊèF¿â{ý3¿åÀ´¼Œ¿ì?_®]ÃL¿ïÿh¶«UâUNASNone?}Œ{œ =?…Õ‡zt?ק%@ô§V?ÍÜ|GJ¾s?ãñThM†?Íé!ÒK"?4TÙü' ?YžˆzŒzj?ã¥n6aè?È9ÆËv?Ø°Ãíª?È9òß夬?Ãÿ×øÕ?¨¾õÑâ?Ý@i'Œü:?µQ´w2Ä?Ù4–v™E?¶*$Ʌ‹w?›™¼S.Å?ÉÅ*²›?çýB"ÿm?¹6Úº_íÆ?̗¾/·åð?·žlùÖ$'3FGL J0737.2-3233@nÚðEwÙUÀ",Ë:%–À9iÃ9À;6~=ó€–?üÆ~a"Õ<@¶ë+g?üòok²Ù¿ÖQ'[0õŽ¿ä½óñ‡¿ê½?á{¿ïÿÆM¸UNASNone?±ÅˆOG^?± «lñv'?æ"Uø¤†}?É|'wŸ¬?ÌËäFB]?ƟÝZ€\á?usϤ áF?€XI¬p?èB`ôT?Á㏊ê
9?ÎãWÿ	¨‰?ÁÈj"ð®?ÀS™#ªò÷?ªðmð…?æŠ1îßÍç?²Ò «=?џ ÕÕi?©oßx'FÒ?ªZ[¿Žå?"BMÏ?éïØoû'ö?²†wdø?ÁªPK"p?¯2|8¼3FGL J0744.1-2523@n*Ûa»û¿æ\°ožôLÀ8u~ÚÑrNÀ;
üaåÎ&?ý
ƒqd]@w@Úæ•÷?ÿ ÛÍp¶¡¿Ú&枰¿å¾3Cû¶¿åþs0Z¿ï‹žw"¤UNASNone?¨ò$ýùêÉ?¬f¡^ªs9?çh7"PW?ʧÆ=?u²?Ì"˜~pCï?È9¨2tP$?8o¸7Y?^ž®¶•}?àÎÑ8mÙ?Ȅí3ÙÑ?Þ\A¡ˆ0?ȈÚ&°‰°?Ð{H¥1îN?°´OŒpa?àj(€Šb?µ³ŠÁ?Í`ò™ùÞ?¯RzŒÆ['?²·ï|õéy?›"Pfó?ç)<ip?´å¦ƒ	?R?ÉýÇOßK?±ñ=vÛ[3FGL J0758.6-1451@m>·€4mÆ@?W´ûßÀ9¤¤ü¤*íÀ;"¥]òú?÷3*#êì@
;T˜Þˆ·?÷©æU´èU¿ÑËÁÀÔǿ҄‹rù6¿éªí_Gò¿é¿jœw^UNASNone?–Ì(u1T?šÜЮ£þr?éKê°?aá?Çã>R

á?Çþ;¹óÒN?ÇU,Ã>Ž?²]Qo?Ý?¹Šu"'U?ãt
6.?ËÉ>0Ùá?Ԁ•Ïú?Ê(ùËFŸ?ÐÝ8Œû7?¶»eœ€Më?áëƒÌÍi2?ºÇ±³_®?Ɨ€¿°dÅ?®Dù[R8?À‡»&—¨?®Né,N=?è¿°7ï;Ÿ?¸¡Ìû³î>?¸óóVÒÓ?®[FÓ}3FGL J0839.6-4133@pRJB®Ñ9?Ô"}Œ.À8†à"&þÀ:šˆŽ¯ZÌ?ýU9Ý@ÜzÛéJ\@™V¸É_°¿hZÀ
¿íø[ª£é¿ëYb…U?¿ïþ/¨0­"UNASNone?~û;ó?˜˜'úgƒ?âçÊƶ¤Á?ѼNŒõÐó?Ù0:£Á?ѳµÍž}?=‹Oþ[;q?g2Rkç
?àÑöëϐ¹?ɬ¥ÄÂ?ÞT¯TaG¿?ɲú!˜‡'?´¸Ð]t6?¡ž…Ê&)?ڒ"Ð;?¸Òi™¢¢?àœdé=[?ºa‹`7Ø?''¢û?^?…×ød4ø?åÿ^¹UT5?À'=Ö©V|?Òé]¡eñ?¿S×Âþ3FGL J0847.4-4327@pxdZ¬¿—»»`|;À8DmØJ¯À:f]@L÷*?þ(˜¨-G@îþ—@ã?þÁyŽ°\¿´Nµ—<wI¿èg×Û|E©¿ï9EÍÙV?ÁY­Ñ	‰UNASNone?ӏ²êO ?Ó¹ˆÞ•Ã¢?Ã*£)?ƽîß(÷?ᬳ½Ç0?Òü''¬cø?­'	³?À+ó~·?¬Ç+¶o?¶ûIZzÖ¾?ìb}ì©f‡?ÄÑȸ´må?Á2²HM¹?¬z'1™Ó?Íj»dÍ4?²ðëöEžÅ?äX¤"¹D}?µ×˜ÝÁ'Ø?ÑRO©gòz?ÇLÙ·j?ÁU+°<©?É}½Â€÷³?ã?G÷š?ÌyԵɮ63FGL J0851.4-4244@pvü;Oag?ïÇõݒAáÀ8UÛ¢R¥¿À:iΐò++?õ¿§@f"@
ð¦z'¹W@€'µ¦•¿àÉIY²›@¿ê¶år
3‹¿êØ[#*¿ã{Ìй҅UNASNone?ŽFì "Â?–.ðÒvq[?»áÿؒ?À=@¡¢w?ì$ëVO'Û?Á-Y¤Û?»>ö¯__?Æ#8 žKn?ÅÖ=1kßà?ÃN'"6>?ç"'ݹ%?˳ś6È?˜ÏY; ÷?¬Ó@`Ìí?Ëø}d»fe?±å¬X,Á{?ä[¬Ð'>)?¶§VÒd<?»5áԖ›7?®Çã
ø)?˺–A‰?Á¯ñ%'ÂX?åÔÕÜÊV?ÁUQFŽl¶3FGL J0854.8-4503@p™¤ü¤*í¿—tR§¬¬À856£*<À:ŠX;*xz?ýã!°SðB@qíVD?ù-Ö|ùÑ?Ó¬¨Üì!¿Ûɽ£º¿æ4È«ø8¿êc?Dä`'UNASNone?`12"™'Å?]•ð݄B?ÛÅrf¶''?Íæ{õ•Á?â
š%4?ÍéÌߝem?!ƒà&?C3rÞ¤–¥?Û3rˆ*̓?É«"Ò¯È?âe.}è*F?É­¦û$ÄT?§Ï'\Žžý?˜¿ÔÃµn?àH=N6O!?»ÄîÛW°t?Üu"Þ?ºUV7Èl?"ÿÂëþ'ô?…NÎ[YB?æM A'²?³îTJ•`?ёh¼ój?²¶"H¥[3FGL J0855.4-4818@pÂq!«KsÀcҢϣAÀ8gQÌ{n5À:vh@Žf?ÿ‡	½=ä@,/±™Ä@7ÒT¿×H1Ð¥¿êtþÙ»7¿è0 ûHòH¿í¨šêbÆUNASNone?p9ìŒÍhŸ?rèBþyöc?Þj±eÈg?у_ã"5?àª3tYû?Ñ~mäMà?F1t§j´?p­†´^?ééëÕÏ?ÁèM" Ÿ:?ÈAÃz>õV?ÁÜ­×jOó?°××ΐ É?Ÿ«j¢J?ݒ§‹"N=?¶ÿÈ¿%	z?Þ7b€×‰?¸- ¢¯Ý`?+a.7tð?wñ傀«¸?æU®˜Pò?À [c"TÒ?Ò×öR€F?ÀhX®êî3FGL J0857.6-4258@p…"ÿCAž?ûP¨È%žÀ8yÊU#HÀ:~ϟåãõ?ø"Íû U@k€´›R¬@ä€ðÖAk?¡
Â0h¿æwúٚn¿ëJ¹4-¿ì'ïHͤ8UNASNone?¾2¦'0äÒ?ºlªÔ—Ä?Øöۄ?ÌÍÖڗ¡¦?à-/ÀÝ&?Î(¼ä×Jt?¾ßö&‡
?™b ;Zý?Ïk›§W}c?ē®g÷ù?äbýeOÆ?ʙ>ÃÈ7Í?¹ú
D¤‡†?§ÝkŠ<?ÔUÇòe%x?´÷DZ)O©?â•Ú^8ÜS?·âî"X?»9Ž…È.é?¥Ýšn5
ò?ؼ 0½?¾S7ë.?àEPöáÅ?¼Ü߇7Ž3FGL J0858.6-4357@p";dZ¬?óN~é+0À8;IàâÀ:o²'ž«Q@Ïh5ã@(ب"H?ý$…(0K¿ÐZ"¿æÆĤNT¿îˆ
Aпà.Ý
6ÊBUNASNone?ÅÁæ£ê=x?Ím#Âœu?»ê?ҁO?À-ÕCò¿Ä?ç+é x?ϯØI¨á?Åð˜&¬Õ?ÌÈ#Ùޜ?ÅbKØ©?Ä`H­‰?å+Vã^ú`?ʊÝ2~?ÅÙÊ ÔÌ^?±6îî²´X?ÌEŠ¨o?±ÀM?ãxKÖ¨"Í?¶˜y,''ä?¶¾†"¼œ?°c†:ù?×üø˜f?Îÿ"Ûö?á)àdì08?Ë֐=|"!3FGL J0901.6-4700@p½o?Rü&¿Ù@ÝÀ»À8 Eð¥À:OY•?úónçê4'@	Wze¤?ýckw¶¿ä3ˆ"¸$ä¿âš¨Éüý†¿èá›Õ¿ïÿ²§ "ŸUNASNone?}í]r"a?ƒ£0Oé^¤?àƯdp2?ÐFÈjò<?ÝúëÁW<?ÐLeQ;()?gL!ùßÞ?'ʁƒ—ŸY?ÚKZšË%Ç?Éu8²z6ê?âРŽ?ɚ·Œ"·¼?¬žg‡8ñ›?šP£‡¡›?á|'С?¶¬6ﴂ`?Ùsãn랬?¶D£¿"?{?¬âŽ&Œ¼Í?¤ó=Æ/*D?Ú¯#}þ¿?ÂçÅFb?àÚE—Ø4Ó?ÂÇ´òYê3FGL J0905.6-4917@pà
å6P¿öÀ³Nv…˜À8†î‰µöÇÀ:¸šs´-@"
¼õ@X‹{ô˜?û?‡ñ\?îê0õ/0^¿é=KR8Üë¿í<Ž"ER"¿ïþvì#1çUNASNone?»W‡;ض?¼è}"ì¯?Ü[G'u*%?ÑE•Ê=Ã)?ÜÎÖ®"¨Z?Ñ\ïøM›û?8ã–F"µi?R̚éj§?ãòµ$'þ?Ì\ί†?Ø\ÑJMT?Ì]8ÓVå?¾Å°['Ôí?ªï+K{kÛ?ÝËґîQf?¶
˜n|?ڂÁWG¹^?¸æÿ`‹0u?JµäY3b?"8W'Az'?éÇæÇÁÿ˜?¿ýUØ/ ?ǹ'²no?½ýD!«lÆ3FGL J0906.0-4705@pƖOv`?¸–º›¡À8²äǕUgÀ:}‹–¡—•?ù"Ÿ48@ä@,9—ÑB}?þÆÌÐ}±\?˳–áÈ ¿ê0";¥Œ[¿îøì»Þ±?§gji͛vUNASNone?Õü›ÏAs?ÔSR»ë»f?§›a³
¬Ž?²"-U®	§?ã‡ûý.¢þ?ÓàQ\ÇX§?¤Ö&)H"?·Ö)Þ^öÁ?ŸAìú¸X?ªw3ôC|Ü?í¸Ž5˜ø³?»÷"žìä?Æ×wœ?±P˜*Ôî'?Ä3Ô˜Ë%?«ýÁ´¶µß?å=-;r̶?¶"' »r?ÚáYɒó?ȑÀ6òd?°\âbä^Ö?»x¤¶éÌ?àƒ¶ÎÚp¬?ÉJ"Ûª3FGL J0907.0-4802@pӓ ٔ[¿Ú¥¬ÍSŠÀ8Ü滋[éÀ:›#ôÑΔ?úßÐVD/@
©¿³´£?ù2aŸb?ïÿ9†$¿ç×e¿èšg!¢<*¿ïÿ¢å8¿UNASNone?}¥ÝFOË?†µÉ¯*-Á?¾25»|5?ÄËÝ\?ëþmŽzÚ?ÅP"•·~?%Ô]Y|jM?K·¹$äB?Ýâæøo?Í/k\ð?á
ZÆ®[?Í1`u­ƒ?´ þ…bZ?¢{»ºƒ§?׶~–"æƒ?µ%m‹G4/?á  ñE`s?·†É÷A8¡?"©•šOË{?ˆuw¯ïÁ?ä4O
%šz?ÂoGUÞ?Ö\ȌÎU?Â;-iþê3FGL J0914.5-4736@pÜk;¸<ó?飺º{'qÀ8/·}°/À:žQY•@!!Ðà,Ñ@="àø(@÷(pa'ë¿ÓÜR>™ÌM¿ê"åʬa¿í(åÂŕ¿Ò?ÏezÐxUNASNone?Þ¸4É+9H?Îóª‰^Çl?²8Î'{¾?¸kJ.³Â"?ܹ—¶°'É?ЎÈ=?Ð$§ipÊ?Ò6%'Ol2?±½šgûÍ?µ/.mq¤›?åµøþHVá?ÑçÄBÅb
?Ör7‡˜¨ÿ?¶"{¾'·€?Éj'ip?®áP•Á®?ÜÿrS¢H?·m•×>Uë?Õäúã(Ë?ÄRœ|"A?ÆñÆ3Gª?Ȅ%'~œ$?Þ¹,9½'?Ç,Øu's>3FGL J0915.8-5110@qÚ{9¿øMzÂ=ý'À8ÞfRDpÀ:ÏÍ"]"?ú•M8`D@õš9ý|Ã@a®‹™%Ö¿ÜzS®'ñ¿í ÙoP"‹¿êOÅóiĕ¿ÎõJ¤mªUNASNone	?ÃLhµ–ÅT?ÀIéÔ%ê?ܜàìÓ–?ΩßOç?Ù¼ê¸a–Á?Ïw•'´?ÂÂ6[¾?Ê«ȺÚ%?ËÌÇÆä?Ì\dWEf?ä\J@äR?Ñ('¥Nùq?Õ¿RÄ$üÙ?´V ýÖe?ÍÓ¢Aҍˆ?¯Í^ü§›—?ÛVÜñ¼b?·p~Ü(Ù?ÓÒ²ïÔ?ŕøˆ®7á?ËïÑÚM­¦?Ì®«»@Ê?Þ5÷`×9Z?Ê]/[.Dò3FGL J0933.9-6232@q£Âã>ÿÀ"`úÛÀ9¾ÙÅÔÀ;" ¨ìó´@jl(T@RãKζ¿×ÎR8œ¿Õ™éº]"_?°ïÒq¿á¤"gÑK¿îÊW…*ªVUNASNone?Ç@Ư"Ñ?ÐñGo%?èÄg<q,Å?ÑÑänï"é?¦¶q|aï~?ºX¥ÕÐ?«;ëäÕ?¸ô¥3à:?çNKG3?ÐQŞc?Ï"fjš?̀ÓÛéÃ?ªÊ40΢7?¡½àÓ{¸¯?ëG¦å?ª'{ï2ž†?¸b
Þ»w²?¤Ôã뚿?ÂHbS`Û?ÀÉòüÉÐ?çe}R0Ï?É+êL²u~?À!©oW$í?Âq(JNV3FGL J0953.7-1510@o~"t¼@=šÿ}úâÀ9Ý8§z¢À;ùõ3c¾?üR:Ð5@
É))D?Û«g𲸭?èz;ì{z¿ÎOo -¿çnS	½C¿ïÿ¬r†§œUNASNone?‡©Ûv·u?"õË#ëQ?íÕöÚ?À×Ęa?¬¹4gD±?À'2~é:?'y¶¥ûËq?Ÿ;"Ýqd|?îå4>ڔ‹?°
u(`?šœÑ¯ˆÓ?¦¬HxñÒÉ?²q»2Á¢?¡³ùŒq?êOV­sÚå?°¬µñF:ó?»IÙ.g/?¨È·öï°?£Xž®??¡ÃÇÚ쟍?íÝ*'Œb?¯ .j+…?žWü'm3?¥5¹½y)¬3FGL J0954.8-3948@p݂ýuâ@&ê@1HwhÀ8¹}uv¤¢À;m2˜Ù€9?õËÔ.ÀÝ«@×-xß@a9n'Z¿ãÒ¼"Ëÿ¿èŸ"L±¡¿ä‹»S8óM¿ïÿ¢Gƛ¹UNASNone?ÜÈìNFoþ?ɲÌà4B?Ô´Žz±ç|?Æm²=Jj¡?Í
nQ?ÅD9	"¸N?¨'k€î¦?°$_KZÝ?èÍÇ`+(?ÁûÿYqâ?ƨHÐ_´?ÂP£1?ܘI¥…Ó?³'¯{¾û?ÖûÁff¤Ï?²­þ¡T?È×ë窺?ªžñl­V¦?Åäðã_€©?°…ªp‰º?å«s8
X5?¹c¯!ãP?ÃmB<k~?±ßt꾬÷3FGL J1002.5-5709@q˜îcŠ	¿÷ƒÆÉ}À8kõœÏ®ÿÀ:O#
KB?öæä‹/s‹@œJ‹¿f]@Â@VÝ1?ÕÆ•^ ¿è	·}œ¿ê1øJ©òW¿êj_«rpUNASNone?t\Û½†‰-?|× ê¡Ý?ÆzGpÃ:E?È],ËÛ1ò?ê8´lT$\?È¥Qµ¶zœ?P>ë x¿>?q_¸]¦"¬?á2ÿ›?ËÉEUtþ‰?݉Á(M#?ËÅ°ÿK›	?­9ÐnÀÁ?™ês¿F?ѝÕîIº?±É3?å]xi§?³&a³ÒF?ËòAµ=^?…Yò–"<ð?Ý´%ªØÕ?§®×˜¤R?஽h#¾¡?·Ï¿ä…3FGL J1013.6-5734@q°ò䎊¿íçù¾ÈR?À8€"¸aÀ:‡dK3'?ü»J}@9[‰"'?ù¯Àéz-?ïÿµÞ¯ßg¿è¹™ÈØ:X¿ëZ®ô¼Å¿äq[ˆ£
rUNASNone?ÊÆ»b?ÍEK±8?ÆUVš8—Q?ËBïÛL2?ãʸª™V*?Ò¯¤œ–?q¾ÞîIª?ðÉuj;?Êuó\û¤?Æ´ˆbÏ.ˆ?é?*äƒ?Æñ4n³¨¨?Áüÿš€?­xR_ÿ+?ÍDºa"1ø?±¿ÍÌ%¨?ä/'má?·xiÇ?©ùN%¼È?¢oY{ŽÔ?ز'Jë?ÉdeÓ'"G?â)úñ.¬?È "jZsj3FGL J1016.5-6034@qÐ=Ć­À	¶	8ÿ%À8¢qȚ8%À:í…AóÀW?ü4_,
@9ΛÙæ@U%o¦+"¿ÕðkhêáF¿íÞ[¦!šã¿è1Xh)'©¿ïþ°ð"g^UNASNone?¸w¦9¯Ž?µšËÓýdd?áÖOW¢?ÎùFù)€Ì?Ö5xY¼dÙ?Î(7LN\?vDlJ£	ç?˜¨@ôVì?çô§ivtª?ÄØ`
?Ï{>÷Ñ?Ä @ojŒ–?Ç(»(¨\¢?­ŽU-}Zã?ßKÊüjçþ?¶Ä*þòŽ¦?Õ×o@é²?µ†S[×ÿ?¤ wª
Ž ?–d"tÖ?热M†ù?¼=;°Lǟ?Ìé,ß`¸E?¹‰©_H÷3FGL J1026.2-5730@qÆM@$³>? µÐ±Þ´×À7Èn4'EÀ9þ¦-?ÿ¾‰öct@\è"ÿV?ü6ݲMD¬¿çƒ/NĀš¿Þ8I5[µ¿é®
Í{¦ó¿éE狏–UNASNone?e[g˜Ô‰?e<ðÜfî?äs
{ TB?Ðù{c]?Öï4:®m?ÐðçQïvþ?`èݱZ¶?‡AÙççõ?ס´Q™}?Ç*kõ8U?ä<ù'«?ÇFd‰»\)?¢¦ŽÒ[j?'?\ÎË?Ú)Õӈsø?½§ÆTj_?áʪ­N M?½ÓAýŽ&g?–‰4xª½Å?'l(åÔ­?ܺ¢p?ÂW›¤+)î?àîeQ'œ?'Š|ý3FGL J1035.7-6720@r&@·€4nÀPBÛÀ8`
z­EHÀ;?zF;†@'ð4ÛÕ@Í£ÈDŽŽ?ûôÆ/¿Ä€ó·áó¿àG±èDøX¿æۛÙS²ž¿îCRªò²eUNASNone?`™*fž²Í?dᩐ\¶i?íøážÎ!î?´T/H™)£?¯hSl³ö?´ÍÖ͝?Rž…¸Ío?jbžÙ·p?ëß
,L°Í?¿¤¢rô?À^›#ÁË2?¿"š,—ÿý?½ÍPçm?~9ÌÙъ?ìï*C÷å?¡õÿßù?´ƒ¾t÷? î'f?‡Ñ­c7ð?yF9â«?íð^œÿœ"?J_¦WÜÑ?«Ð­iÇ?›¶ˆó3FGL J1037.2-6052@qõ"œwškÀT*#¿ùÀ9ûkEÉ8À:õå†6a?ø‡,å'?@
Ââm©Q?þ£ÐqÇîl¿Þ7 <$bO¿ëŒíîÒÓn¿áûÛxê«
¿ïÿÿ¬?…ôUNASNone?¦žž±!š?²¦Oå$(?ÀÞ0¾9K?Çu[¹ï‡?ê^ŠU_"?ÉÍ¡÷ò¢V?q¬aÍó'?…²D[M3?㊨>-¨?ÊQØÚMç?Ø£þDKÖ¬?É÷¯šo¹ã?ϋ­`s˜?°"|И]p?ؗç|çè·?²°·ö÷Ù?×¢AÓÝ|?´pGŀQ?¼(±ñ{?©?—Ŭ?ÚЭ²Cqœ?ÂÁ፞Ö?Þ%P!@/¥?Á/ý5£·ê3FGL J1037.9-5843@qåz–¼¿ÌèöÎþÖ4À8T=;"À:c?J˜ª†?ùhðÊ-
O@
Hy|î"?ü]Bf×пæ1QÚúHA¿äl(
Ôèìl†!Rò¿èJGy€
UNASNone?†JQ ìu?'k÷÷…õË?ÉȈ"úé?ÉÞÀ'4?é4µÊð½"?Êi-8/?R5úXÏ;?t袶E4?ÒÖX¥då1?È°AA?拸°!%Ë?Èœç0"?À1ø
œ&?§+Pè0s?ÓH`óus‹?´îUöRÄâ?âOQ'ÿ_0?¶F&V·nÆ?¤&#×Z?\gòöWJ?Øõeç¶ôÇ?ÃúãÏÇ÷û?âDj©òˆ'?Ä:»H+ŽŸ3FGL J1039.1-5809@qã4¢3œ?ÖuÌ}ɯÀ8ÖmpEã9À:x‹îN?ùžv*úÕ@ü²ÎHøÂ?÷'\ÆÕfú?ï՘KÌîA¿à'ß\¶(4¿æ£% Bb¿ïÿá…ÓiUNASNone?`¢†âŒC‰?k0Žr¬2?ÊÐ%,%aª?Ëè÷mb4?é;T.R?ÌãJù"x?'œ08ì݋?Gº[¬3ðl?áêXa¶Ö?ÐbñüÃ{Ñ?Ýí7É5t¸?ÐcFª#ç?§
î\SNJ?–RÅÛ?âSìÑ1?´ã;æ–û?ØýúZӆª?´VÐ.:Ëú?‰¢ñï•F›?"ëO¥Šb©?äۋÏN?ÄVΤi½=?Õ{ÐÑæS¾?Ä(@4aõÕ3FGL J1047.3-6005@r½<64¿ë–eÒ°À8Yóv"Á›À:;°ÂF?øF&ñ}@$	-{8[?ü<|Ã$¿Þ®ØÑñW¿ÄòH'ú¿êÛÞLž` ¿ät+º²²´UNASNoneT?JQ/³©??}…ï$\á?Ô{Æý\Ø?Î,"ê?僇ßjB?ÎðŒJ€?l˜þŒ?¢¼[Cþñò?ÐÍõ;Øf?ÇPß>cP|?ç#Tï³Lü?ÈÈm@a?·Œo"ì"?¢†}k^"0?ÐÀ"È
ˆ?³<FT'Eþ?äÿ'ÕK[·?´ìÀöF³?¹mc²p'é?°g-Ë'ñ*?×_#úUO?ÄhºÅ?á"ÁŒ‡F5?ÄDï!R3FGL J1048.2-5928@qý³Ð|"¶¿Ð¬@$Þ0ÍÀ8Esvð!fÀ:7F°¾yM@…'5yß@¾ÅÍÿý§?úZ¢e›e?ïϯ??¨Y¿Öºèÿ]mÄ¿ëÊÿèƒ¿çoi¡H(}UNASNone?¢$@#¦1?±(
Òâ¦U?ØpɛÏpˆ?ÐïÂ×ÍÁ†?â¥W/Ýäª?Ѹ+‡Ý?yé…ËÄ7?˜ËìIÆWá?Õ
ïïK?Ë«®ÔÚÀ?åEd|ryÓ?ËÿêoM?´å
…?¤Š(¯VÉ?Ò>m"gÅ?³c-^8Ã#?äD•oz?µxÙyõô? teø"Î?™´!ȯè®?ã€6(i)?ǂ¯ˆ‡ä?Öÿ%"nã?ÆŸKÃ3FGL J1056.7-5853@r	7ޓž®?粓€zä£À82Òò€»|À:°†ˆD݀@ð+Voù@š@QT?ýaÿI ÛB¿Éb_CF¿åÌ<>Ó-¿ëå­X_´é¿ïÿ¡Ïý6UNASNone?'õeüƒ?™êÿEXT!?ã³s½·?ÏîJÝOãf?×yǺ~ÃË?Ϭ=yɬ?-‡¡W«—Å?T…W¡ã'?ëœÀ'í©ž?¿¥¬s*Ü8?Á…›Ëón ?¿§MÞ|z?±ÅÖtNÓ?¢Eì@Üõr?â®ÕGywì?¹«>ûú¾?Ö1{oüu?¹ËEyÅð¦?^
¼‰üc¿?WýUü'®?íÚj	µ¬?¤xŠÑA‹?°¶Ù½Ša
?¤'6Á3FGL J1104.9-6036@r#¹#¢œx¿ØæØ|-xÀ8脹7ÅÀ:~¤™@3gáe¶@l\õyi?øáY÷˜'?ïÿX"ò2¿Ü-vÕ8E¿æ
L|/{n¿ï~@ÝÀºñUNASNone?#õ•"qå?#ïŒ~g ?æK)ÚG?ÏH;ðOoŠ?ÓgZK
y?ÏHnO¥µ"?{ä‰Õx?/Ÿ;r$ô?çSÊgÊË?ǒaUñNÕ?ÑW‡R¦Ã?ǒŠnŽÅ
?öT3]?|Æk'A?ç·ñ¬m?µòFƒ"Uû?Ð=|_¾«?µ"Íšg?k'Ôë¸Z?f¸ògˆ…ž?è6eÁdÍ?¼»l¯"w?θ h¾½é?¼¢žö²Û3FGL J1112.0-6135@r6^Ý)5¿î¨0 ±»ÏÀ7Ù³×2]À:C6nQs@«húp@Έc¼=?þ#ÉO"¾¿ÑåÅÊ­–¿æôþǛµ¿è]—ÆìÊ¿í£ç?·"UNASNone@?iw¿"Αÿ?eâë+øôg?ÞɈpa?ÑÄ}KD?àæ[§ù=?Ñ"Oý?8­œ¦µ??WƒKZǶ?äTezÔcÁ?ÇbIB"¶A?×Q	£UNÏ?ÇfHn,
Á?£øº›Ãøš?™NPwµ?ÞHÀ0œ07?¹#¶ÕÊ ?ß8({ëPµ?º—Ð<þiµ?ŠÿÏ´å?IZ†´¿B?ä(G~êu?»Ä¾Õ>Ÿà?Ö×r‹ƒî?»~Ó¡Àì3FGL J1119.9-2204@qGƒ[Õì@B†6`åÀ8Ώљ»(À;™tÆ{yô@$7÷E¨@Œgƒò¾N?ö
óxˆ'¿¥øV9]¿ß,âP–¿è Âb(‹¿ïÿê#¨YYUNASNone?§­šÎŸÄï?­Š2>÷Ó?ìïŬ}E­?¼~`ž‰÷N?©V
i‹à=?·¥#iÓ?ƒʀd˜?—sÈgðå?îÝVÎà¥?®È¸±µU?šÏ–>¿¹,?§TÄ?Œ÷?À1!¢«??«t²
²
x?çþRX'µ"?´'ëqæ?¿«)ùlBá?¬ü{Ÿ|~?—
è‰:"?ŒÃv͖…M?î…e¶6!w? %œµL^(?˜E`°̬?™Ä¹xµj3FGL J1120.6+0713@oqÝDU@NW´NPÅëÀ9ÒñÑsûÀ;åû¤P¬Á?úèE‰L‰@þEjÃB_?ñ›±‰¥ZÃ?ïKT
¡Í¿Þ~G˓R¿äH§Á¥|Q¿îÃËV€bUNASNone?˧ÐD*·'?Çkz©Ù"†?æø{Ûòåº?Ëò.mŽû\?°ì€˜c)?¼l¯Ó$7?׫hÁñVW?Ò
¸v²¶z?áü"XÖÖÃ?Òj´ëk!#?±n:1ƒð‡?³WR;IÚÞ?Ì9·('á?²ëSJlò?ã#4à¿3È?ºj—™?Ç9uT?µ'CæÁ'?Ö¦Êhþº?'«#3:¢?âijZ=®?ç[ßÐ,û?®žw/H?°C£ÜB<3FGL J1128.6-5434@r0˜ñ/@z	Ì1œZÀ9eDܨâãÀ;cÚTtÌ[?÷9ÞóëË@
M¢÷Œ¿@
l…E¤¥¿á×i'òÛw¿ë+fiþ¿ïØڌï¿ïÂ
H½ÞóUNASNone?ÂMü8ړY?Äéˆa¿?ÝöÒ	Ϋ?Ï^ߜ<‰?Øâåˆç¨?оº÷ÿ?¯agšYÈ?À\A‹Ø°y?å[‡+ÛÇ?ΡÀ0ûÊÛ?Ñ]›þe]9?ÊcyõÐyu?ۅëàÔo'?³ÏÑ®?Ùã@ßÂdß?´†þK`?Å-¦~ÒW?¦zEv§â?ŸÇb{WYý?›Y÷
-?ìÒÑøÚ£?³™ò6†?±w—šU!?®}&2K3FGL J1128.7-6232@rYŸ±¿òÓe7'=…À8º5À¬-À:¶î#;n?ûó"vøYî@|CÐd[õ?ù!֙Õ(¼?ïô`9¦"Õ¿è:5+Âå¿êg…î
‡¿åáe<3¦ºUNASNone?™¬}i
Ÿ?ŸdÀh†ª?Âð8óu(¶?Æ|p£G?êvÚgme?Ǽ÷šPCx?pýÝ\Ôc¸?ŠŠå/Ý-©?ÏÈ6€î¢?ÉRðÌ.ö?çëö¥E['?É@L!©®Î?ÊÊQ-<™?µ1î÷QÕ?ÍËXÅMt{?²p¶öwè?áÚ¥:aSº?¾!2rfkV?®²6œ+º?¢ãè«+?ܼK5ñ×?ȇ9ÿ¬?ßm.-öˆ²?ÇYÁ¥|k'3FGL J1208.4-6239@r ]'ýuâ¿É¿{*˜°À8ô!-wÀ:	÷;5`4?üJ5XQ@©·6ì%?ö̼†®…d?éòz1Ìß¿ÖÀ}xü–¿å®€Rî¿í§õ'ùoUNASNone?ZÓ®Kq?`ÙÍâÄ~?Ùϵc1VJ?Ñ"ًPg?ã
»ÂHµ?Ñ(½Dy?^œR³y)?}—èñ–þè?Ó­n{r¢{?Çöð4Ô|¸?æúµU?ÈÞÄ á?˜(bhC?ŽXm—¯>?àl&§×-d?¼!"0·`?Ý¥,0>³?»êq¢2æ:? «¾ý~g?˜Ú7#7vÿ?Ù_ÿ-¸?Âj!JŠ??âfA4'=?Ž÷Õê3FGL J1225.9+2953@g$ÞÊl @Tðñ¾ôœõÀ9wÒ4jkÀ;¨Öí·ÿ?úOó«³Í@>¥"8äù?óJCðð™?ÒïXæ© U¿àW¼ãÜÄù¿×UXÂ8õ¿ì'ŠyÉ£*UNASNone?·|ñiœ?¸WÁ"g*?ë2%MË?ÂuvžÅ‰?­Ã´JØ ?º©<vx?ÖJ¬]i£?Ó>cVþ í?ágˆ·`j?Óãu?»™ÒpK?ÂËÎ
*fÄ?Àë­Ãþø?©¹}&Ð?è5Z‹kE4?°U€xRƒ?¼}ЉØl?¦¡ˆxFk?×á¨>èr?ÃKýÙZÿÌ?áÒòv"`?Æt'"{Ò?¸MMËOÃD?±ûÆk£"3FGL J1231.6-5113@r¼Aò×s@'»%}À9fƒÂ—ÀÀ;uëGWL?ûšÄÒW{<@ĂLuúX@ó¡­k¿Õ:æÄ*ù¿èAܕ†~N¿ï礉·¤G¿ïØ¡—>ö`UNASNone?»Ôüݓª?ÂYô£½4#?é8©æ*"˜?Ƶ]P?ͪ?»ÛÑÍǔ?»žCE`c†?"*/4Dut?ªfYôŠH?ìaž²b¥?¼ÕñkâjÁ?·èƒ}[Íy?·W&õSßF?ÓugR?²`lû>t?àS©'ad´?µÖä1?ÇÇO'sž?¬£Ñ¬X|Š?•­D«å—?‹ú	d"ö?íÞêÐ1©^?§%kF
?§:°¦òÝ\?¢Ù'D3FGL J1306.4-6043@sKœ¶"Œ@±]''À8xÅ
»ªÀ:¶…F%~??ÿƒ>ùºì{@™;³4uS?õrjùs¿º¯&&bóÉ¿Ößë}ù¿àì6GöÊÞ¿ësiø¥²UNASNone?ràªn?yEa"'qò?íüÜëà!?µ¦–:éÐ?­ï›õ,½T?µ?RrÊލ?S¿ú‹|ö?k~ÊD!oÞ?êeçBÕ?ÃÆ?ÆDoÜmÝ´?Ã7DxØ?¥Á5
Fy?š4oŠ­dŽ?çóù‹9?³ÎhÁfMÛ?ʿ̐5äÓ?±T!à&?'¬ücÿÓ?yLFQäÀ½?êH¦ß\iÍ?µ"!ÖÅØ*?Ų£'ÈÔ?µ4·½u€œ3FGL J1317.6-6315@sñ¾ôœõ¿á3Ïp;ÑÀ8?M«"}©À:g"©GŒ‡?ù9í|o½'@a'ÇMµ?ûJ)©ò'>?ïêu^üº¦¿ã^,æ#é¿è&lX÷F¿îgùt±¾æUNASNone?r"÷HÆþÉ?unˆÙ?àÅP"Ï?Ð';Õ,+?߈!ÓEË?Ð
H8?2CIïý?P^'ˆÁ?Ü(ø±Eˆ?Ë?­…ÂT5?áé;=ùùy?ËCč,D£?ž‰þCÅàô?‹Ù]T_"v?à¸}Ýþ|×?¸(ó"¨?ܦd_ƨD?¸C_"e?–Êv"J?Œ@]­¶×?â'"ÑÝ?ÂTd8hç9?ÚD1k¶r?ÁÿÆ䨣\3FGL J1329.8-6109@s8ҝÇ%Ä?õÕ`IôÀ8ÔG'‡|À:€ŠÔÚ¸?øBw÷]o@Åßó›?÷pµµ.£¿Gctö/¿ÝÓÙ"à¿âõ‡›D¿î¼P3°AãUNASNone?wWÀºƒ¶??yíÂ6•2?ß	rëÔIƒ?Ðc‡­Å"?àL— ÓÒ?Ðy áŠ0?¢²çÁ?±Ñ»ëbƒ?ÕY[I?Çžª0à–?äL$âHÊ?ÉBÅSÆÅY?²Ã{m? ìòàÇì®?ä¯ip©äœ?µÒèR©~?Ò§-Ít°?³™rµI?Æ¥w?°àÜQ@·?ØuÔªïÐr?¿W¾õÞ±?܇XÑô?¿Ð¹Ñ.A§3FGL J1350.4-6224@s[ZîcŠ¿Ôy4¿zSÙÀ8i1ÈÏè
À:sî,ëñ?ý"£'–Æ@B%±ŽX?çµçF[ë?ïúT\ü¿Ñ¿•_V¿â"°õ·¿ïÿò|ðÒ¢UNASNone?}1"ÇGL?ƒí¢PáŒÉ?á®Ç¸ÒnG?Óq3W2=A?Ü-ª;>ÒV?Óz0Aõÿ7?Aä?mÉ?d bß\!?×pìøî?ÐO}R½È?äCB
ì$®?ÐRðÇò7?¤×Nv?–ÁÙò¡É?ä:h&mdw?¶<<ï:š?Õ
+Ø;fã?µXø©'\?£Ï0D»N?Çց锂?á•ìŠ&Âã?È
¿¡`u?ÚZ@ãv?ÇÑiص}i3FGL J1358.5-6025@sr	ԕ+?õè|4gÀ7䐴Ê!À:Sýå¶?ûI"dvL8@Éf<J7@Çþ†Ù#¿ÒVƒ¾Õ­
¿ä˜Ñ1$T¿è'&›É¿ï-9†ßW¿UNASNone?q%¡dg?w7"Y$b?æÅé{–o?ÌbDÈLMQ?Ò/–ƒCØÙ?ÌJH˔cC?r¾ðöH?†ÅZÄØÁô?㬶P¬Ý?Éj†Cµ@?Ø[›³Fâm?Él¾D
6%?¤NyÈK??• Îö>+î?áL¹‰ÕëD?¸‰²\dÈÍ?ÚÜÉý ?¸ƒèÓ0¦$?"%–¨*œ?†e¿P²?äY´Oto?¹q¸u¾À›?֖ó,áx?¹:
@/3FGL J1405.4-6119@s{!Bp?ҕa¼­žÀ7Ґ[,À9Ëp£×
=?ÿñ´â@BüŒX'?þ_ÛÛ£
¿Ó‹
9ÏYš¿ä]ï֫⋿çvº 5¦;¿ç"vµû
^UNASNone?E(\?FæâkÉ?³z.ȎÕ?¹ÇÁšýxÿ?í‹u8¢.?¹ÛØ9ƒ—?Mò»ŽN?rq=Y·ôV?ÛZèQÐ?Êÿ$1?âK•(["?Ê(àî("?úC`¹?uï+?ÉÁ[Cô|L?±"P|,|Þ?èŸ×àw?²C{ŽNÿÊ?{-ßU¥?wNôù3Å?Ú Ç"ð?ÀYÕûÁK¤?ây˜÷S×?À…
³³3FGL J1411.8-5743@s˜•1ã¨@èX¡ÅgÀ8õil«$À;Î70ö?øº¢OÎ@'9"áV@áÈ¿Ì߿ŧä•o¿ë·Ö¡-¿æ[8'R3¿é†¤9ä/óUNASNone?¯mŸà£&?¬mcX?×)峬K{?Íí0çH(?ât3(§á?Î
FWI??²×íÞ$`Å?¸[ñÇàBð?Óôê¸"Ûî?È.ˆ£R
Z?㪌è*ò?Ê6p(AI?ÖOo²õI²?²B°ÉŇ?Ô¸˜¸üs?²^Ò&oCç?Ô÷÷"›Û?²±(.?Ä°/?£Œ?®Hê$À?ÞeJy÷öÝ?ÂYåØãVÃ?×B§nh7^?½×›æì3FGL J1412.3-6635@sm¹à`þHÀê°]*}'À9†ŽVox^À;@ï›2÷?÷U¸ìp+6@ò©nοÁ?ú2IÂ°¿Ýy¶rËØ¿âi·š›¿åœ0õì*á¿ïÿéåèUNASNone?±òŒÌ¢«¯?³Â¸ÖÇ?ãj¼MÝdÇ?·P;Œ[?Ô­ä1‹‡?Ík!L}N?¥þéI.ÈÅ?²®ÝwYÔ
?âÀàz‡bØ?ț"9Ü 9?×¾aáËa7?ǖš2"-?Æþl¿?¬³¦ìíØn?ãû@¤Vë?´Cî˜WÒ?Éò 3?®
K¸U?ÈUôQ'?³Øý8*?á&H7n‰T?ÀºËQd{/?шu‡ č?»ÂJŠ483FGL J1447.3-5800@sÜï4Ö¡b?÷®ITèRÀ7ÿö¶«"XÀ:…Ћž.T?÷¢!Ódk@'
t­@Ýë´½·¿ã€ÌÝØ|¿éy<˜üT"¿ëøcb"¹z¿ê¹ËÌ$cëUNASNone?¤;"ºäá?¥Ô¶œ©^?ØW³jÙ?ÏW$xå?␿ZÆüƒ?ÏþVÇ?§¢.í³F?¸à͝žç`?ÛƉMJ?̚Ÿ{…¬?àü[	Ì~'?Í7'µeÜ?Á´ûÄ)sy?©DÇ¿Ìž?֞BÄQ¶?´ÀãË´Kr?àC²m"zG?¶–´=û×M?¨Þ¼%ò>Ï?™Û«õÙ;X?ácÑ2?ÁoÉ0Ž|?ÚÓÿ³ŸT?À.M8Û+3FGL J1456.7-6046@sÚVlô!¿ø˜}õÏ$–À8I)B©DÀ:.^¸<?ûCç@ìY@"óoMì@'åÆmã¿Ãö'àªáQ¿ë^}õàS¿ì"f›YQ¿ì17î-ð~UNASNone?wZö[É?z‰˜¢ÚGÉ?ä¶Ïú)?ÑY"¬Îþ?Ö6cãïÔf?ÑGÀP—C?/ét%¦?¨–{Qåm?à¨HÙªZ²?ÍÒ¤¥ýÓW?Ý·dÍ_©o?ÍÃñ»Å?¯åîâÄҏ?ž,þÛx?Ù^féûaD?µKoýB_?áRmœÖ5?¶®4í›n?˜>®%%P'?"´÷Š?؞8¬·Æì?ÄÃ9ؕȃ?âîî8zò?Ä·Áå§ðJ3FGL J1503.5-5801@sûX£/D'?Þ7_úfŽÀ8–—†™ãÀ:5œBÁE°?ù§œSÞ#Œ@Øٗ
ž?þH»eqHî¿Úù> #Ìc¿æòn-@f¿æ¯'ùš¾»¿îڌ{×oqUNASNone?>ù?åáò07?¤Yœgø?®ütñ ƒ‰?îBàa?y?±<Ò©V©?xáí½>u?ŠëXhG?ÆC²%¬¸?¾O{"3»?ê=O›?T?¿€m¸¿¿?µÇAÔÃÅ×?¤åŒñs)i?ѹ™Vw´?´&6c`1?äúø¼Kj?¶aál–©[?¶¬Éd&/ì?¨ŸHGšrÒ?ÎojQÄ??¸*¬Þôõe?åŽxæÈó?¼+§;M°3FGL J1528.3-5836@t"»â.]á¿û"à¢l¦òÀ9~e`¬éÀ;_Þ+™á¾?ý}©^2»>@ë.QL#¿ã–/—ÐÊ;¿Ö؎ŠO'R¿¤ëÄüÍ/C¿æ!ڛB¿ïÿÇí%CUNASNone?âI±$DTþ?Ø·Œó¨²%?Ðù­<º¯?Ó¸\_0X…?ÄåàõyLî?Î/Ë£ê߉?¡~ÊÕ8Yh?¾þ`óT¸á?ס˜GBñ?Ô#í)EA?ㆈØò?Ôí/øK?ÇEK®¹?±HHîî?ãÆ.Ö:?¹¬*Ÿêê³?̂›•í‰?·`î3¥J?ÌZWXU‰?Çâ°R Ù?áƺ`T€Ë?ЃxJòøû?̋'U§L?Ë­°þ;e¿3FGL J1539.2-3324@u,%ãS÷Ï@1ˆÁDŽPÀ9.èŒEôÀ;š^x[[p@(Ò·rrŽ@;«Ò(+¿ó…¦÷ú"?ïþ°Q/â?ç¡eº]Î+¿Ü>S"ø䔿í‰ÕB€òÈUNASNone?˝³Q՗9?Ô^ÆE"'?èxsòz?ԑÅSñQ ?"ç/ö8?±ý"‰p?¤ÈU—J4?ÁgŽÎ¡ž…?ì‡^Â~E?ÈÝÌac1?±c¶_ h½?Àböi\­?·-¢µ"ƒ?§fƒCP¤{?é®°Ï÷'?±Ë^ºO?»\ÖÒD2ì?­b¯4
Z?°;(Ū*?¶ö«Åªñ›?ìKô}ˆ™"?€b`¡[?ªÊfœ!dg?¸$|?¼3FGL J1543.5-0244@K¯'9*Ä@Cs7âÅ\–À9ÀÁœ¬tÀ;¬U^f?ö|»WYƒ)@±¦˜/·(?þG;N	οҙÎeܱO¿âÞÓüýþ¿ëù+'Lm¿ïÿ¨×¥ýUNASNone?悔>EŽ}?Ç2zýK'?Ñ%;.œÚ1?ÇãrF€´?YÅM€H?Ÿçh(ü(??ß	YJ#1†?ÈêOù:$?Ü]$Þ6?ȶôt¤'ð?²fjFÿÁ?¯É'Ç3F?Ûs6H>˜?·%OKãZv?Ü÷‡P–ZÑ?·`)ÁÅd?¿¸䅚^?¦¦ËiÒ?Òؚ¤"}5?ºZhÚ~)ò?ãºz(-Øñ?ÀázÇZH?¶ÉÄ,C¤?­ò|ÇÌ3FGL J1552.8-5330@t]$žDú?ÓkM
ìÓÀ7å-c™ÑÀ9ùt,!Æú?ÿþnÞ,µ@´Š­B˜×?óÕ7‡€½U?ïÿŠºZH¿Û+4*©ø¿ã¯wuhž
¿ïò]΃AUNASNone@?DÆ2˜§‡?Tt9·µŽë?ä´ºJƸ;?ÑÙë'Y¬?֌(Q&ˆ4?ÑÙ®»FVó?+²ŸŠ|cœ?Lz?‹Ñ'?âñY"à?ϾMÉ:Ø~?Ú×gîðf?Ï¿C&˜?ŠÝ`]åÀÝ?ƒUl"—Ïs?å3^lÂö?¹²›Õ¶3ˆ?ÔÂX#ŒÆ?¹s
ÎÎg{?y|éÿˆ±?u•ë†‰3?âvEVò?Äpò¨‡?ڗ#:GSú?āouîÿ!3FGL J1557.0-4225@túB¤TÞ@ ¹mmÁ¤{À8ÔÔ{øÀ;
Ìhù¾?÷ÇV%{˜@þý~Ԝ@HåY‹Œ'¿ä Ä+q%¿ë[4aº
¿èM9Þaä¿ïÿT,ÉFUNASNone?Ԕ‰Ñ]!ü?Åñxäq¥?Õâïkûi?ÈL$&F¦?Չe?6âš?ÉÀ.FZï›?´K§ü\6?¼µçñS»?æfÆàb?Çv83·­9?Ì?½wÍq?Ä>•ÂAZf?Ø%É}®Ðþ?³× ¹?Øçà˜Ü¬é?³Õ
"Ýý"?Íä«Òé3?®èå÷¥d?²©;?J¡? ^î· A?æ½A]Ö?¹s×AŠög?Ë·a['f?´Ýצ…s!3FGL J1601.9+2306@CDÙê¦Ò@Gx($xÀ:_ñ÷ÿ€~À<@žReþb?÷6(¦I€@ÎÝћ¿¿Ûäúr™Çß¿èÅ&õ?Îkƒb0ÝÕ¿çD uRº¿ïûõú KUNASNone?áÀˆÎÜç?ØP™BCû?Û'ñ22Xï?×È…›‰?•oÓÞÔ?²\zƒ§Ž?ÀŽ9®'i1?ʁ9j–@?ê2»â$C?Ώòý?ª›[%+-?¶9¢jÓ{ƒ?Íp›ªý¥?·üµ­n)?å Obâ€?»E7Ð8'ÿ?¸Mɚ¶?¤ø6skå?шÍË×Ý?Ì ;Ä^¤?æf¤Y2›?ÍâCقšŠ?£	WLq?±š!f3FGL J1622.9-5004@tÛMüã¿Ñíþ`BµÝÀ7nœwškQÀ9ïÇßþù@ T¬)¿@ö¡æÅ~?ò¬œ2Ñ
¤?ïþ¼ö\í¿ÓfIyàZ¿á">‡ïø¿èªs£UNASNone?p¯l˜"×?w­®—g?ɚ1´Þ?˓¿h…pÝ?éxˆy®ß?Ë× "·
ã?B¨»ø0&Ö?b‰ï9†÷à?Ó¤gO–¬?È
õŽ?J;?æ)")6î!?ÈøDl?ª? HÍg¸Ì?'sûz.yÔ?ʵDk­ÍX?²ÒŠ¬¯e^?èN"?´9ԆÑì?"úÖ¨÷¸?1ò¡
)»?×ò®Jk¡ ?À\NG@?ãfؼçs?ÀljøkB3FGL J1624.1-4700@u•¿ðEx?û«>ËÌÀ7öك"t—À:ƒèäö@ÏM%²—@eý€ò"@¬.õ5÷‰¿àHÅ]0¡w¿î6ý'½\l¿àY®eƒ'¿ê:"39EúUNASNone?Ċ¾¸zw?Ä'ºÇzR?ÙÇÚDDîâ?ÐÞJ{Ö§?ÛòÆ_~a?Ðæ%–4nr?£ë²úõô?¹™œ'?âþë	É?ÏW!!'?ٖfWʍ¯?Î^óM§;?Ād^Ï£ñ?¬GÍT{U?؟*·Y–?´°IOnv?Ý £Ôq?¶,½J¦•?¦i-\·¢?¡·h­è]~?ÞðpŠ¨?ËUƒ[CÊ,?ÞBJ8¾d?ÉÕÇF·ÐU3FGL J1624.2-4041@uI&Á½¥@'x³puÀ8f­VœÀ:Â(4Òo¤?ÿØþÑ×£•@l%y6LÃ?õep•x?—{^èV¿à^]eX@Ö¿å…2ƞ¿î±Èe› "UNASNone?d
>q¯?akÄÛÔ_`?çönÇ?ʄñ!dGY?ÑÓ¬¥?ʆÿ4Š"?~îGò–»?‹Iù¹'mŒ?è)kÃÄêP?Ç<CŒ.×»?ÎbÞ´ÜÂ?Æÿ.>K,?›•1ä1ðö?'kÝNW)U?é¥5Ц?±šÁºJ¼?ÅùIŠ¢J?°@a'Ž‡?œê'¥¼7?‹ä~?´"I?èä¹;Ӗ?µÊ̙Oÿô?ÌÆoú%?µ/ç¬<ç3FGL J1625.1-0021@+Âþ`Ï6@?Özúr!†À8¸@ƒ}ÎbÀ;ež8dË\@+ÐïòÝ@ô?ß n?é…ìï_§c¿ËUO
¿½­mÌaB¿äãaó Yοï¯8gOšUNASNone?Ky;åN?S^"eŒ¼Ö?îÜ´
-Uô?³'Ø"²O?¡ÆÚm–+Ž?³|ñ϶®"?`‰¤wûÁ
?xŠÑ1"?ï'Î	OµP?›ÝŽxµ?‹*Ž»æ?™QT³Þ?™"ÿy­®J?"ÑÜyË?ì–ùÉ;?¦–žÚ:ÿK?´î0SJ¼N?£¾+DÎÀ ?k8ÎþÄ?hÝ&¢­(/?ïqÝ6©_?äŠòrx÷?Œº~–ô²?Ž§êœ"Q\3FGL J1626.3-4406@u%øa¦
E@ْ]e5åÀ8®•Í\>ÅÀ:lñý2Æ?÷Q¾SEÎ@
lÞÃo¾@(qrÂÀ?à¾ñ¢šO¿îÍfØ°7¿¹4xJZm¿ïÿ¬Lh}1UNASNone
?£¹
Ë<i?±sÌÄ3S'?¾þS,7	?Äh¬·ó¬§?êä¤ÊZ7?Ç} þ[š?µ¥*XÖ?~?ÁèiŠ…?ÜHßZðšû?Щ×!‹tk?ÞMÖÙÕ'?ÐM¬'Í÷?¾Å±ß»?§#¹5¡…?Ôº_"1'?´"	3|ç™?áÊðJ?µËXâX¢?¶ÿí ?³ìD%?Ȩ\›–Œø?È49Z{"?çhÛfYÒ?ÊŒùÝG3FGL J1641.5-5319@tԻ¹M"Àh†
 zÀ8·Â,_Ú[À:Òð§h[?ü–$,?Ö@ªJkÞö?ÿā6÷8¿å`ý6ÞÀ¿â$¿²²ð-¿ë¥ÄD_w׿ïÿ†™v'UNASNone?Ânm? Ræ"©J?ë_…í9{?Áš;]E?½½àÓËä?À*L<Pj¹?†eœB–‡?–hd泜?åIÂâ_|?ŐaÈ{S?Ô¹MY,›?ÅK:ùqh‰?¼m`OÜ*ú?¥oÁc³Ö-?å5e¬c?³<›…æ<‡?͘zD8ö?±£TLÂÆ?¯xŠÆ3?ìÚCÆý?ç&W!.`?»Sá%JÌ?Ë÷ȟX"õ?·–!Ø©3FGL J1643.6-5002@tÿ÷—|À"¬_nû`À8Ì£²!OÜÀ:©>Ò£¦?û:"ˆ¹@tš{ìµu@ƒ@;ÚL¿ÐväÎKR¿æ
vrf鈿ï4·¬¡€¿ÍˆV8¤iàUNASNone?á[?"]1ü?ÔD¹t?Ñs^ïeÖð?Ï£LñöýÅ?ǬCÓ¿Š2?É牳Šé?Ô[bÃ,%?Ò×ÖÃC,?Â/_zAÅ?ìv#"?áF§ð"}?ÑU¯§+=À?҂î¢Ó"ü?¶ùÔýŸ(?Í8°œå?±<`E¦µU?Þà¹,?ºŸ8ìäºÂ?ѯh(4}!?Ã/§,¿C€?ÉXsÇ7?˳Õh%??àÒ/sÚ!?É
:ði3FGL J1645.7-2149@vay=Ùc@.D£çÑ5À9'E«Û»}À;om¿öûu?úôõj¥»;@ç²ãA®K?ðž)¶²¯¿Ç¯¾(''¿àuIó`Â¿éï¦Ä$‡Ÿ¿ï¤Ñ¦ÙÑ¡UNASNone?pÅ;ºöÚf?x¡‰s†0?ìñ'~tÁ?ŽK"¾Í™?¾"¸\ìT?Ŗ¢`\ ?•®`i(ט?«¾Ô
5^I?ìẺiôÈ?Áh]É®¯.?¸fšf#Û?¾(Gzbâ?ªsð¬N•e?™ŽECý"ä?êÏû¥á-?°£u*"?ÀûÃæTÕî?¬ÃDäÒyi?¥†ME[N?OAüÑUÿ?ëk/y·\?¸(¼×rIï?¹ãa9©z?µ£:P9®3FGL J1650.3-4600@u<Ãa@O¿îxd•«ÎPÀ7"`X/kþÀ9ÄÉ«?þýøKU¾Î@â¬2#?øwïzÌ¥?Ðs"k(±¿¿àÜù6¦ôæ¿åïólìõ¿ì
ŽDUNASNone?<ÏØ"™*?:L}[ñ?ßÖàÞL5	?Ð#n–p'1?àõ•Õ'V?Ð$p·°?Elë C?_"ù?ٗ}0?ÇH¾Bèp?ã/5zwJ?ÇSb+;?±£s¢ª;?uØ`èѕá?åk'¹BV?ºç&§¨
&?ÕI›Þðf?º@˜cV?K}ê$w?Š@÷Ís?ÔãX\3?¼f
Ãð?å€Ñ )T?¾
­àÍä²3FGL J1652.8-4351@u[¼w¯d?·‹Y:À8]–
˜à6À:_yv
£W?úÎMÖL¨O@«}ůÞ?Õ	u…ÏI?ïÿî]ýG¿²§3zʯ8¿äòç
2*¿ë¡ ۆ'ÆUNASNone?"†Ç-ù²? çÃÊRŽ?Öi¬$q¸?Քw®—úê?ä3·´+?ÕøàãÞ5ø?"w×?²˜l÷ œâ?ÎL6¼Ç·?Ìò$ƺ)?çÔ~"GZ%?κUÙv¹¨?®Š`¬Úñ? €o.q°?àC6¼°?·ú¿ìHª¤?Û¨}|ë[é?¶ëÏ:!b?´Nnßo8?±x%1sÖ?Úŷç?ʛ?Ü?àg➐?˼%-ËÀg3FGL J1653.6-0158@0ž=æœo@8ì´Zåÿ¤À8õŽŒöÀ;†"éß,@Gú~¶¿D@þ4x؄?ý'úƒ"I¤¿×'^:â˜Ö¿âFúR
‹P¿å?çx8­¿ïÊ8&¦Ì¢UNASNone?'Á1í&q?Ó—²|cA?íáìŸ?²',ž—?©`gHHr×?°v/úýÄ»?yçÕÎø£\?‰Ò["Lb?ᆰ*ø?¢»jr€íc?—Ž5GØ9? qV
|"5?°d-êAõ½?¡Êm»dN?ê‡-@ݞ?¬¤r"Õq?»biƒ·X?¤Çºosaç?8Ò½:u?'_´"xo;?íI7ðcCŒ?¤«S¡Ì4p?±¨ø6•?¡ô&¯ª‹i3FGL J1654.3-4907@u!ÀD(NÀ°WK@pÀ9»Z´|À:Û¾	»j¥?úp¥+H-@\fA''–@×B¤•K+¿äëÌÂ:øy¿æÓ*ð6ð¿êË×qÿå¿îµN»-UNASNone	?'ÃÞ-i—x?'Õ×Þ?ߋ¨«1²?Í⣨"!`?ßÞ8c'?ÍÝõ&ò?†èëo‡îß?œnÝìnY±?äĊ>0	˜?Æe°$¥O?Õ¿¤(#­Y?Æ@Q¢Â?Ëë3'N)?®Ç»Q<—?ړŸ%œÂ?´e²b_A?×âkA%¼*?µrÔù€æÝ?­ìLF¤x#?´¬ªKž'?å>%GX?¼±ÉÂä?ÑÆ,sâL?¸·l¡!Ó`3FGL J1702.8-5656@tÆ]cˆe•À"}DUGZÀ8*ºŸ£ŸÀ;'8|HP?ýŒBn@K}u ¾g@ûaŽ»D9¿ßÔâJbyÈ¿å2'¤¬¼¿èSXpj²b¿é®!/>uËUNASNone?Тç«Þä?…‰¶–à?à¼ðò	åž?ʇbŠÙä?ÌÚöh€«Á?ºYÊqK?¥d4$áuÏ?°¨ºèR§?ââÿ'Ñ?ÊXqOê¦ý?׍{FHË£?É<îÄæ{?ÜLOŒ5ل?³í_ˆÄ?Õ½ éÌIH?³ltÞӚ?Ëìûºi?­ûsK('C?»üPF&'Á?§Ñ×|Š?å¼Ð8('°?»" ØԆË?Ë–üJkà?¶°F0S&3FGL J1727.7-2637@v}T!ÀD(@FœÒ3>À8–ØÐN,À:¶[Ëر?ýdÕ÷ú@ A]òz@k°ªØ0X¿àëïhò̀¿éýç"fh"¿ï†¾7U#?¿ïø0ðŽjUNASNone?ÐÏÉ{/_ƒ?Ñç€sù\a?Üù¾Ge-9?ÑV}±pÐ?Ò6x=ksD?͟,-j"?˜V: fÂç?¢Ùªo(\¿?㛟!kAF?ʕð~Àƒp?×C^#F?ɣۇ ÇÞ?ÅYZ,(Í?®h€‰iý?ÛXª'*Mm?·ž §¤×?Ùú¨m?ž-?ºG`ðÖ?–DáÖrô€?Œ#%óïEF?é€0š›'?¹U'PÐ??Ç6¡ZØü?·ö}å3FGL J1729.7-2408@P÷[ìá@AêÝYÀ8z«°óRsÀ:ÀÒ£¦bÖ?÷¦Zøt"@iÀÆY@8@üÞßHûG¿×Ù^ˬ¿ê…..€`¿ë±N¥®ö¿å·nðèNÍUNASNone?ÅK'Ïä¢?½ãw¢çº?ÔÄNG«¬?ÊM^šz?àK3dã¢?ÍaV=p%%?Ù2"ÖÐq#?Ï7o	Us–?Éú»ûUÈî?Å(¸Zó?ÙÐ+"ªe?ʈ´ÁW9?Øè…Éá{?¶‡z u¢?ÈÜ6ù'ÊH?¬$՗2È?Ú©_ll¹`?·íÇ/uþ[?Áµþ¼J@Ù?®!Ž|iÖW?ØMª0&üû?ÅåÓs?Þ×Vq³â™?‡³84e"3FGL J1729.9-0859@.oõHìÙ@+&æS†ÒÀ9Bs9³õÀ;9/bÄw?úþø–T?È@
ÜTÎczÏ@må|ñî¿Øê(@§t¿ì6'üDK¿ïÿ´h¤ž?ïð¦ä/êÔUNASNone	?ÚÁ™LJV?Ñ£J0"-?Ý?^ÙÎoç?Ñt´Ìqލ?¿ü -¨#
?Ó½5×ä?횔QfJ?Ãü6ÄÔô'?™Ÿ}l¾?´†—ãÔn½?©‡.«Å?½+¾BÎù³?â*4Þó=¶?³Þ>pDÁ?ÎCNg^úª?°*ªZÖwì?ÉÞÔ|?¬°€¥"ü?åò*²5p ?ÐF¾»â­	?»¥[.³ð?Ì*h
?Ê©‰'å‰?ɍ;Pžøw3FGL J1730.6-0357@3ͽ@gÏ@/în"ŠzÀ9Ä斢nTÀ;gæ…·?øðMÈà¯@3·«þK?ߣK¥¤¿Ú–ú©T?¶k\€š«N¿â_lµñû¿îT'BÙiUNASNone?†ÿ4ív|¬?'Pô»mö?짟k·?Åò£Íæ?·çäfóxb?Äz*8U}"?†ßµòÕÑ?§Ò(:[5?í|Ÿ§tƒX?º°'	x?¯ò•­¾_œ?¶VŒÈýŸo?´¨‡Kc1?¢ÒÓI.?é–2{érã?±&LCŒÐ?¿JÙiº?ªÐ…:pÛ?«²Ø¼Ô#?§˜ÔÿŽºÊ?ëK£Ì×!?»´9Gšü½?¸¡u:Üé?·¾Œ^3FGL J1734.7-2930@vd*Ã") ?û6«Þ?»ØÀ8•—Œy§À:zŠÊɽN?ù¼Á"Šf @¡œò¿?ö>À?°uñWrb¿åýu·¿ç$ù³yƒh¿å¶$ÿ‹2pUNASNone?î'Ú
5?Åðڋ»wK?‰½Š¾€"?œ\ù©m?ê­e^€v°?ÇãqÛö²?֌mf8ÞM?Ó¾Ò5s¡l?®42\@C?°­#hÞÚ?âֈé½ÌÖ?Ó?Îã]¹?ÐO¦YË?´ºfuÂ}l?ÃpÁwb¡?¨ *\Ù8M?âûü™AÐ?·M®nAZ?ÒoýØ?í‰?Àw¡ÃžR?¸—'8ÝZ?³-8€Ùžý?ãÆ.#˜í?Â&²¨Øý3FGL J1736.0-2701?àWà[õÊ@iÏ!:ã+À8¼°³ ¬À:œ÷½;_R?ù®WÙÛ©	@
1î¯ËŠ-?ùmª*5ˆ£?åËñ»C¸g¿ç¼—šˆNe¿åuµ}"š¿ïÿáïôšUNASNone?†¾L%ŽVÌ?"#lúye€?°¼"¿cå?»ŒŽü»??í£>ÑÚ)?¾ԃ-ç?wN
SOíQ?‰üÄßnj?ä~K|?ÊH9: ?Ö¦ªœÈF?ÊHvsÆÚw?¹8AõžLí?¦å³u?×´x‡‡²?µÓI0E?àþ÷r‰?¹¤x ùó?˜ÚpãA|^?‹htVÁÿI?â9Òt ?Á…7²t‰?Ùÿ´&þü?Á3
­¨K3FGL J1736.5-2839@vr÷eýŠÛ?ýn'«?´KÀ8—cW¾,÷À:´²G^?þqõ0K¦@/° ?ò`àëgÿã˜YþyC¿ÛΆXÒ²¿ïÿñÉ 6[?ïöúNKx¶UNASNone?Øû.d
	†?ÔÞØ?ÏP%ýÄô?Í[â*¯Ë?×\Ðô?Ò=4¥|‹Ü?ä®hÂRó?Ö*y樚Š?'"É@ÔÆP?¢å
°™ú?ÕyáçLÍy?Õw~¤x?ԚܜFZ?³ˆ‹jìü‡?Óì&`/.^?²'è)‡ó?×xýŠÏI?´€¦>Ý;?éɃKÝÉ??È[N¦x?ž"XÖ¯ò?µÏ¯Ø[ë?ÅEn?Ææ´ä;Àð3FGL J1737.9-2511@B¡µÇ͊@~HÀc1þÀ8O#—´½À:ÙXÌIð?ý
Ä<°`@ªNò]U@ÔäÁ5>ü¿áð²Q˜Æ¿é8¢=­	¹¿ì5Ì>ïÿ>"Ó—uUNASNone?Ì/1-ðuo?ÂNc4
I=?ËÔ¾|')?ÊUŒ±fpø?áÿ0dØÚ?Íç'Ðߘ×?°VåÀr	o?¶7K(à—?à !>nÇ?ÊE¬í>?Ûªà ?ÉäpA§xo?Éኯ7?°ÛFŸN‰?Ö{ªa:®?¶Š¾ú)?ÝX"G6´?¹Pšì€!i?¦Î'×"î¨?—ýÜJ7?ã%Ä	†ÞZ?¿)¨ßÌ?ÖÚ§'ÿ¥w?¼äíÑ€´3FGL J1740.5-2843@vy>Õ(?ñVWûi˜À7kŽ#CÑçÀ9Ó=¶CôL?ùIA<‹@³¼Òì™@ir©´¿Ï…Xþ㏠¿ç»³Ï½¼¿é|ç´Q"T¿ènÜ*ÝUNASNone?NRȸÞ`!?SQ‹9®ž'?¼.o7Äõ?ÂÙô+-ÄÏ?ìrfÙ)È?Âé"'±?•ŐiÏ?¤éÑé´x?ÕN(PûðJ?Çùw§H>'?ä¬jñU"?Èm™`•?ªX ¹}?š‰Óï?©õ?ËÙ/VÎâ?´^ʬ.?çd>¼??µ
²ÇÉr?'ÐMxÍìË?ŒYïÿ›½Ú?Ώ8b.m?· Å&®'?çͺ!þ?¸piS«G3FGL J1740.5-2726?妟ê$Ì?û»èÿ2z§À7ù/‡­À:3µ«HÇ?ý§7è¥@1	½@ÛçF÷¿Ùv.ü¨î²¿è{+½ÑÞ¿ê'ôRLÔ¿ïÿ›o÷M™UNASNone?†ô…eÁ‰V?ärŽy»æ?ÊÜÅ¡@ ?ÌâÎà´á?èí(9©²?Íg)-•uC?nÆA³±áh?"u‰x׸¿?åƒoâ"?ƕ-òh<?Ô»"¸X+?ƔÆNã2™?¨Gw/ ?›âÁƒ†'(?Ô ¥°!(}?¹Kß[Ÿ^?ä.´#wøÈ?»¸âJ¥Œ{?ƒ¤]O%?{2¿'yP?ãÍåºÚ!š?¾(•¹wÇ?×ÇŸÒ"2?¾K<*̔3FGL J1740.5-2642?ôÞ i—sO@û¿¼CÎÀ8ÏËRyI˜À:µ½Ñb^?øºQO}ì•@ìG'd?ô4đ?¿±ïGºU†,¿àìi9i¿æIæ¯æ¦×¿ïe­¾ê‹úUNASNone?^
r!.B?c;y
´?&?ÞëÑ*¸}?ґúuÂÔ?à{<Ú¾?җ^Ÿg?iŠÂSí'}?ÅS¢çr°?æ%<Ã%6r?Ê ÷
I?ӂpõ
·ö?ÊsŽT'F?§…ž‹—ß?"vÅi֝?äÿJmËδ?µ8Íwj9…?ÓÇ°–ï›?´&Ô#¶2?•3Œ]'l'?‹`…;Ç?åÍØA÷?ÀåBWcà?Ó¢û?Àúûe+N3FGL J1742.6-3321@v>p†nD¿üdóºw_³À8)+hc–¨À:wfÀ(yœ@kä'fI‹@˜?&†}?öñ ԋÝï?ËÄÇ>\Jó¿á†ÿI\ül¿êôϺÜ¿íô[L
lUNASNone?A"—h[è
?D)Ü‾Ž?ç¶ÌÀöL?Ì'X¡[8?ѿȚÉås?̨_­s¿?4L—;ÖqØ?S¦¾ñ}ìC?æ…;='?È»³<¿šÀ?Òðv_1èX?ȼB-ãV·?Ž8CâÛs?ƒ
÷ÝhÈ?ç'.m€t?µJ»¤iÀ&?ÐÀ%Š…è=?´³Û^˜?')ýåà/´?x¢WnïKÔ?è'êQO17?¹è'®e œ?̑¶Üe8'?¹ªÉ'3u3FGL J1744.1-7619@sѬ<žìÀÀ6x›ÇqC9À8"{?;2À;]"mé§@W±\®×™@'p\"y?ó¼†=Ç5ß?të¸cËäÀ¿Ù&t;™½¿åÉâܦ'¿ïÿíkÜOªUNASNone?ƒê¥ú¢½\?ŽŠüÇ_ü?íÿûÂåé?¸A=3)I?«
VÅ(ò?·9¦¸Í‰Ý?l.
²í9"?†8ÙÏ8
æ?î!9ÁË?¯oŽ{=@?¬,¸´{?¬ðYÄô$å?¡¡&ú¬?•ñ-øXÛù?륓Çbø+?¨
	âÏûÄ?ºÎÃk>J?¥cúSàq?"ø'_'Ï?|¸²]ג?î#ë÷ÎÄ?£™I>4Š?¨ƒ9^ƉË?¢̚þû3FGL J1744.7-2252@N8C=lr@
©‹XߕÀ8¢Á¾{Ñ2À:Ò('fvW?ý 'b"s@^ߥ—~·@÷§üÞ¸]?¸Ø>Óp¿ìZV1ò¿çRg!]ƒû¿ïÿ'Õ/FêUNASNone?µ7í~Àš?²²íPÜV?Üß@Mü'?ÐTm÷dS?ÝÒÄR×?ÐrÍÎê?‡åÛhP!?•‹<^ñ
B?ãO(|w?ÈIC@ʯ?Ø¢†àÎb?ÇïÚ2©]Ñ?ÁŠ|AQŒ"?©"/^L¦?ÝK·9%K?·›
Ƃ¥´?Ùï
¦1îž?ºk>?¤Ė‰þ?'{Neð÷?æ?…w뵺?¹PpÃqÙ?ÐÿÜ}ecL?·6¬	Ð;3FGL J1745.3-2903c@v}Ò½<6¿"" 
êÀ60•âTôÀ8¥ãÛÝ@%{‡ŠÎP@	ùù€´ñ?ô¡9óÁ®?æÚcY\ë¿à'î}î垿ç–Ûñz¿ìk]ãyÑAUNASNonep?Ž4¡Ud?m8»Þ?ätÀ	Â{?уßëÿy?×gœ« ö?уËCob?"²"LÑñ–?B<ƒdhÿ?è1ôo®V?Ç­MÐõS?Ï3'ån-?Ç­ŠY÷ŸÎ?d¼q¹»4m?eOn
Ø4¨?éØì×M?²fQË?ÈIZÛåÁ?±úi->J?5·"ͳÉ?AÔËô.>×?ÙEåÂUÄÓ?ÇùxzO?ãZV:{g5?Èp¿Ñ03FGL J1747.0-2828?áÔG '¨;¿¥(ÚûÊÍTÀ6¦¤Gr…YÀ9Æé]ý@úÁC`Ó@ÂÁ†º?ûtS5G¿Ä34	òÈ	¿äÅHEWç·¿è]xãQÛ¿î"ËÝUNASNoneP?}…ÐÛ35ž?'¼Õ)V®?°ъK²?ň/6И?ëDˆ)ç¨?ÅßfZæAM?`k6}u=?{^k\NÁÎ?Ù¼8…Î%T?ÉoZbØHÆ?ãx©âoà?ÉvtÑÈê?¢©|àTAs?œ"²à,0è?ÛRQ1ì*ï?¹.q|Gå?á,?™¦q?¹ü¾æ&?"iº·Ú Ò?¹y:—Ú?ؘbՊÈb?ˆ¬'ÝiŽ?ãb'ª[3L?¦n͸ ®3FGL J1748.3-2815c?ìà³3ž"¿Å#rö"À7âÃ2ðUÀ:h)qéQh?ÿ'´µÔ¸©@9›
²ái¿þÞ²G»U?åiáypô?ƒ4K´ýÙп͝D¬q&¿ê"ªúƒÙUNASNone$?ÀŒŒ
A…?ÐS@ù¶?à3[C?ԅ)¹C­?×SÃDÞ¸?ÐùfэÌ?'Ü(Ù Ó?¹ŠõJŽ˜‡?Û²®s…)/?Ö]Y@£¿?áÇub?ÖxÜ]4Ñ¿?®§Š&ë³q?¡Ì&S«&?à2³W-\?¼²gÁë?ÛŨ€t.Ú?¼S=åL÷C?£fßU¤zF?´Vï:ŸÀ?ÖìîèП?Ô$ó¬Ä ?ãSñP?Ôç­
ºËC3FGL J1749.2-2911?ȦÃ"Ôì+¿êתv`¯À7Í«û›í1À9®"ñ¹ì?þÐâ»Ìtb@
ۼܿ´?õ$ýÍð
?ïíßvȉF¿Üن±+þÙ¿çLÞ±ëcÖ¿êÅùé‡åßUNASNoneD?2¹/øéj?2å)W¶ÿ?àJ	åÉ ?Ò*O…?ßgiGœn†?Ò*°Rݑ?;e³'B?W¡[³Òí?ÝÇoìi£¬?Ë/õKÁ½?áÛSXëÇ?Ë6Lë†êò?ÆnÜÆF?"Z'[??á#ÐjIÇ?½)BáŒþ?ÜˬS´†B?¼­–øé'?{hAò•Ë?|Á'Úþ	?Ø	u¢="?ā8Sí—?ãĤFªü
?Äfªœ½»(3FGL J1749.6-3133@vcpâÁ*ØÀ×)9µ-tÀ8²²eByøÀ:u'OÐ!ì?úHDºšH@
ÒòÖ¡¸?û|½›+•¿ßäk•ádp¿æîrÇÑC¿æŸPµ¥ô¿ïÿƓðÖUNASNone?͍FzE5Ê?È£ä#°	?¡óèÍ?©,ð\	ý=?猍¿t?ÉêKÓó&?±§¬âiø?½Û{-Rƒ`?ÔV+Œäf?É6¸ ˜?ã½_Yý@?ËÈ¿aZ?ËYQ©¬h ?°¶ÿl3²u?ÑӞê€ÇÅ?±
fïÂ?à?Ü Tö?´ƒïhÆôx?ÈAšü¥}å?¹œ{Þþ¡³?Ê!4Ù²z/?¾_j±Ì?ãgL
jû?ÂvXµº¤Ë3FGL J1753.6-4447@u±]ÌcñAÀ"Õ5†Ê‰üÀ9dßý+9jÀ;cìƒKy?öPrß­*@
·²ˆÓÏ?÷Y˜1å€M¿Ùl°f:¿Û¹Š¹	ª¿äT*\¨€¿î·(ðmUNASNone?qU!ž¸\C?p[ùJÆ?åuC†\˜?Îótá?ÔÐ$lÌïb?Íù"Ç8òl?ŸsEÙ˜N?¥ºßé0 ²?äӓŒ$]q?ȯE~ê³ù?Ôa¤Ž¹«›?È)cP§k?¸i"ÃÔ?£j×@êÚf?禌×WU¡?³zþ'ÖU?ÅbØ@¿{?®Æ¦·8ݕ?ÅAör–Nj?«†ÖHºLâ?ãΟ^vœ?¸¨\Â!s?˃ŒŽ›J?µ0dԐ3FGL J1754.0-2930?ÜÖ¦ YŸ¿ýÊÌ&´Ÿ¯À7çå7&ݺÀ:2ËÏvË8?þ_¿c×ñ@[çÿ@G$êp Ï¿áÎ*2-¤©¿æ¸€"åÕ²¿ëÁþ¸,VË¿ïü»8¿}ôUNASNone?Š45À5T?ÑPðÜ߃?â
€;yj€?Ñ¡ÔL
?Û]Û'-?Ñx@þÍ?d'ŸY¡¯?{¹¦ÀÇl?åϙV³?È_ÔÛ7{?Õª¶ŸV?È\<C#v5?³\C³NˆÊ?¢U¥ |µ?Ù§!‡¹ÍÅ?¹‡øjàÓR?àÀæŹH?ºïÞэ|.?˜÷-ôgu?Ž…þ/ŠÊù?᲌¯Øì¸?À©vô¯_?Û·-nà?Àˆ:683FGL J1754.0-2538@?§ëkôE?µ»Ä¼²ù<À7æyó$÷À:T9ܚ *@wp×ÙpI@ÏôTüÊ?æގ¿‡%4?ïÿ¸$B`¿ÑRôþˆöM¿âaåí"¿ë#‹²(›UNASNone?Â…"ñ¡'?Çß݃Ï?ÞÊzè¸:Í?Ôc†0ãZk?Ø)B…Îô ?ÓÀ'6ù
?h±5+?'VWcGQ&?ԏ±`Ý2?ÎSCÖd}b?å ÊÄ\f?΀Væ«?¦Mg°$?š.MßÔ)?á_ïG‰ ‰?½G<b,´Ê?Ú|·Ã÷ºl?»­ÂD\?£beNw?›Ò!\2<Ì?àp"ì6?Åزÿӛ•?ÝtÛë}Å?ÆÁ÷503FGL J1757.7-6030@tÐ,<žìÀÀ1*$š<À:W"'iÑUÀ<;¶N?÷6&:&l{@{QZÀè¿óñF×Tæ?jiЬ<øÇ?ßÏ|k¾¿Ï	K®)I¿ë¹KÕZSÍUNASNone?Þ¢´!Ž,!?×y/QÊâ?ß5j'/?ÖЩÝϓ?¡?
zUýˆ?³ö´%å?Ï=ê4¡k­?Ò±°LJco?âÃx½MÅ?Ô!¢ô
?Å´3Œi]F?Æj<˜Wõ¬?Ð	ó÷Dç?³Úí¼I?ãÓÓº!G‰?¶Z†SŠ?ÀœÉ(ñ¼?©ÁãO"ÑB?䞁´éè?Ð
'mƒY?Î'½DV7ß?Ë낊™€Ï?¾¼wÐ
 þ?Ä·HT{ìZ3FGL J1800.8-2402@ÓW>«6z¿ÜíWœI!\À7VIÿ''ìÀ9¶0©ë÷?ûepÈ@½ÉljÁà?ù1%'¿Ò
'ús¿ãÈÓÉ@PR¿á_)oÁë¿èᏄ—ÔÈUNASNone?H-™øá?QQ÷âU=? óÞ1ï?©S-Ÿ2bO?îøu{6¦²?©ª´¢/¸o?Fâ¡ZÓ½3?do›eà¨?ÉÏ%í╚?«¹ƒDÿ?é†}Ü0¥ª?ÂÀ?'`×? ½è©Ñ…Y?'G|
Û
"?ÉJ­NL¾?«è´#	6?êÎÊT{?­É•>0B?–ÜKn¿ˆ?–Z?cŽ?¿¾% W/?²Ãm~®~?ëQXó§~?¶b6 B`Ö3FGL J1808.3-3357@v`÷<ÉÀÚ\¢˜EÝÀ9w;ØbçÀ;DŸqIï7?ø
.j€@oÅz¤6?ôž9ŒÈZ¿Ö¾l$žù^¿Û‹ÿÅ*¿çVïó9ëV¿î°¸ë!)NUNASNone?"Šívtœ*?""¼åÂ:ô?èﱆ…ü?ÊPò'E?ÉÏÜ7T‹?É桽m«õ?¶omTÜÓ?¿g3®FÁF?ßÒ|?C'?ʁÒ¹5+?ڑ½Ík…J?É)âcÄ??µ (!o?£¬ôæ«F?èGìÑð?²MUX`hÅ?Ä,Lœ§‰?­'pÈòF.?Ïk]šîSb?·×ïJdÄ°?à>;‹ß|?Áv€h^ϵ?ϛ´5•n¬?½ÌBW¬Š3FGL J1813.6-1148@2OµIùH@³Œ|z¤âÀ7ÁÐ\¤EÅÀ:¾­OY?ÿ"VÔxß@¤[©ôۊ@¸½ÄMc¿ÝˆZá'Ĩ¿í7úb˜b¿å
V<-E¿ïÿYƒ÷=[UNASNone	?ƒ öqs5)?–XCQ/?×ù¬yˆ£Â?цU.¢Ég?ã´¥éuáK?Ѭa3;øV?g/ÂC
?Š²êÌ;†}?ê:¹*êà?Ãõ{êémÓ?Ƹ_jéKs?ýhߪCí?±)"§`Ï0?¡	"žÝÞO?ÛR¹XZœ?¶ª_H¿K?à1p¾æ˜?·?§aöÌY?hµ´ÈIô?kNÉn¥(Ÿ?åìj'"?Å÷~mx ?ÓõÀmMk?Åçt…»3FGL J1823.2-1339@1š¥ç…µ·¿¸€,5=$À7jf¦'GÀ9R[Æ?ùJšèùÿ
@䓳%±À?ýwã:"¿Ø`ð"¶—¿à¿Ÿ×eü¿ä5†‡8¿è"†¸ýsDUNASNone?P¹þ×À~§?Q&`7@?¥°8î?«ÜÞG3]?î¦WþÀž"?¬°}sñ|?Db³²˜4?]JcxBµd?ÊjòÉu²?¿—m./Ý?é`*œõÒn?¿½Ê¶Àe<? bŽj?gÐïÖ?Á©k¨ûÁ?ªVŽ$d~Ñ?ê|/GÏ?¬žh²Ùòù?ËL¤š­0?ÈÕÿSÌ?ÃPƒ¯KԂ?°p[ï¶l\?ꥄ¯5v?³ÎÚñߨê3FGL J1827.3-1446@1ud0+A¿÷½¢!þW‰À8ˆÿI ÛÀ:•ýʛš%?ö'Ò€@
'Ü®—,­¿ía'ÞÒo	?çtÝ̃¿Ï(œA8ž¿ßH–3€¿í³rB_ŠUNASNone?¹l¡
¤ÛŽ?ÆÍ+@Ä3?Ø?áÿŠ¿/?ÑqGl¶l?à²zÞæ÷?г¨-ý?'ež«œT–?²m@›"3?ÕFöšî™Ï?Óô3À…Ã?äÑW½+Ðt?Ôa—¦ƒt?¯à!¼=Z?ž8"ž¤?à{~2?¶_h2U?Ûÿc>4U?µöíˆé?³ÜeÞ»p?ºD 
®³ƒ?Ó%î²´‡?ÐÝúÝ?ä	-éäÌ?҉Ýeıª3FGL J1831.6-6503@tŸ?¼À6gø"»ì«À:‹†³
&À<e»À5Ö?øð+oð@"˜ýgtX¿õÇlãË¿å뒙0yV?Á•î¿:èß¿à8ƒÝ£<¿í…̘IhUNASNone?â7¡"X'?ÖßûÐ "?ÚϏçò¿?֞,˜'9&?ˆUŞ+ƒÑ?ž³,N"æ?½]ÑV4+?ÉÇ.ú[Œ?ç°ºDsÅ?Ñ9M=ŠëO?Ž.cˆÞÛ?Äæ/Êx6V?Ïx}»?³qÃg[]?â".ã)h?µüÇ´ä™f?Æ;<_rÜ ?±/‹ròñj?Øöcf¿"?ÑRBw,µw?ݪý‹1·?ÒGLöÀL?¾7k"‰?ÉÎ[óÏ•3FGL J1831.7-0230@<u^á6ç@	Ó˜K$ÂÀ7àùx&'KÀ9ÆõkQ‡²?öÉLÌKž@»PÒ@´þh{>¿ç"=ý;ª{¿èóAç½$¿êF$mƒÍ;¿èõM¤E£UNASNone?'nÿÑì
–?ˆ°ŠÜû>?áŸKà?Ӓ.O>X?Ü-ðß°•a?Ӕ­"ï_ß?¸;/c!?ÃL r?à}"Y•Ñ?Î×:`cJá?Ùó¶ït?̤x}ZA9?¼ƒÏÊ?¨B³Vg?Õë¹Å|Á?·=ð.ù?ᇣ˜ˆ\?·Ü~ft©µ?ƒíÁq*r?†lrŸ"‡¢?ÒðŽiÀ¬œ?Åu¿‹õ?æ8Å[˜?Å×ї'q¢3FGL J1839.3-0552@:S¹EÅ¿‰ÕÓ0¿ À7±EˆÀ9SÓ[\G)@cªpCµ@ûÊ"x{?ù"ü(¯÷¿´Æì`@&¿Û̕asû¿ä徸âà
¿êës§¨·*UNASNone?&«`Áž…?'<V›@°'?Û4çwÐÔ?ьµ› ‰\?âd!Žwk|?эۑ½¼?vqžälS?1Æ¢% t¢?å"X†wçI?ÄI	ÿÉVd?ÔÕNjöC)?ÄIzg¨e4?óË+UÅÄ?z¡vkõü"?áW(?ý_?Àño"?ÜÂ&ª1?¿æaŲ+?`tï äl?c _ÛX?ÚtÏ
çî´?Ãn€	ç¿?âµ#‹k$:?Ú¾%YEˆ3FGL J1843.0-0359c@<mCx$Õ?¦µ¯`À86(ï'µÀ9Éh%ƒGH?÷Çy8¦È@š#WH?õÑÄ ÙSï?ÛÁòu¿Ý˜˜ÊLü¿äh˜pàÎó¿ïÿÕÄčUNASNone1?[ð·Ø§ô?f¨¸ü¬­?¹8»eÔö?ÀnÓeè*?ìË`%WY
?ÀG§Ÿûõ?nßِï¿?‰¶Ñï¤|?Ì8×>®j?Åú'Īò¥?èÞRªVÃu?ÆQL¢§?¡	Ì;'?"Ñ»G>"h?Û«<m¼}?µ°Õ1«µ?áÈÌ`Ê	?µ¿(fä? ï+_‰­?¡ð†#Øá?Èj"àOƒ/?¾ÿ™–¶À?èå/Õ6&š?Áºµ¢+i3FGL J1843.7-0322@=çáüú?ƍ¥šƒÏXÀ7ªñÀ9À¨á59ž@"Ùz/F@'Ý<Ü@CÕÖᣟ¿Ü;š<#>¿çòµ0Æ=ß¿êmIçՑ¿ïÿAHl"UNASNone?€Š\þ?†
®
UE?Ä]½ÄY7?Éþԉš¥?êžoño?Éná	?ðJ?P/!»j//?hݳI‹\?ߥÉÅ,"›?Æ큃Ëm?à%ŒŒ?Æ÷骟Î?±àè@"‰V?£Պ¬µ{?Ö0†óë¨?¶Š(üGiž?âºJ´uy?¸ÑÖ¸N:8?'™vŽÏ{?~T͖žõö?Þ¹-qď?¿V$D«5²?àY˜‹ßÌ?¿¤§ÿG÷…3FGL J1844.3-0344@<˹M"¿ÂŒæÃCBÀ8I­Ï±ƒ›À:9ºHf?ûîÍÕý£@j#²Œ¯¦¿Û´ÆVø?ï÷sB܍N?Èé"}m¿á_ûÎBÓ¿ìtĚúÝUNASNone?š¥õ'?²R¥™ÇK?؎¸ÆO"?Ò<åŠ?âã{|p‰å?Ñ؍vF¢š?B¾X4Ô?²oe]ÝL?م¸,¯	"?Ô/ßß*të?âÁÞ¯c?ԏÀ	ØÑ4?š‹Èfö*?'Õ"z$?â1k°lø?¸o`à7}?ÙômR/Ãf?·ê!Â`-?˜C•äuÔ?¢;/3îl?Ýi@r+'®?Ñ0Ӗ'ç?à‰Cz?ъ×Qvû3FGL J1848.4-0141@?…fîW¿¼Öpd—gÀ6ã¸WÊÂ1À9‹‡Öùvy@¥cSa|@´Üú‰?ÿSqç£è¨¿ÔàÜJ»‡¿çÈPó¿æv×·%_z¿î"Í]UNASNone?_SØË/?b>WæÆE?Í×q*´{?Í®ªm¿'?èzz,æ{¡?Í»
ö=?0׊:#?R;GïÔùã?å<ü"."?Æ= èq ?ՁÐõG8?Æ>ót»´?¡6Id™w?—.Ý(êáA?ß/¬GU?¹ü×½A?ÞÆ'%Š0?»ªÿü^ ?nR' ØÌ)?l¼ê7?Ün¼¯D1?ÁMÞpx ?áªO=°?ÁqL"½83FGL J1848.6+3232@O$¡œZ@-| fèlÀ8ãÌґÀ:]vfœí?üÑÂèbÒ@{þÔü?þçÛv]ÕH¿¤\¸råµ-¿éôsH»Ê¿å¸±Òø¿ïŸaæ`,øUNASNoneP?ëÓ&^ì=?ÂIÈl5?p:ǐ¬Å?{0â»[õ¹?À1'YþîW?Â3©œQ"%?ï5ço3n­?¢§ÌÎ7/?{Ö[;0?Œ{ˆ––³á?'M{JÆ(—?Øû&ïÑm?ßÛÿ¾"ÑÛ?¶ˆ>Y/ª?Á»6ݍ²?©E>ù'X?×]"¦gL?µÛ¾ÿ™?åöÚÈ?ÄTÂõg¹?¡Å—ãW?©ÛW³é{à?Ñï`+©|…?ÃIIÝä‡3FGL J1851.2+0423@Bh"pdìê@d}€^_1À8'­K'E¿À:T\Rn?øè뗾"@1+¼ÇF@šO'ã—¿¿ãŨM!Ø¿ëÄ7Da¿éF	Ï*N¿ïÿÚLÅ´UNASNone?»ØC€ª?»‡2®—àÌ?Ïu$ªi%?ÊýùA4?䧮ec¦¨?ϧɺˆ×?§òÚ,î&?¹ÚÞÖúþ?àȬ@]ãü?Ëúü­s!û?ÛpL9¦sD?Ì{60Õ'?½YÚYp?¦Æpï"w?Հ"o;q?µù"+¡€Ï?á"z§`È?·Ñ¡q4Â?¡e:b'Úœ?–!97c?à¼۟¼H?ÁÑÏ?Ü[(ünL?Àï«Sî‰O3FGL J1857.2+0059@A<YÈÉ2¿êçLàƒböÀ7À!)Es¨À9wúÊ6˜?úSÀý
Ø @.…fîW?õRtK×Cô¿àû[4û¿ß£†ŸcT†¿áNnokÀ¿éE1çwcUNASNone?R]HØ[c?]
ræ,¢Û?¯\žè"‹¹?¶ã>=#ÿj?î‡SK?·fxk9ú?¤*½qðþg?µíµ?Å./k.pÅ?Á°	tÂÃ?éqÈNSè?Å`îcÏÿÔ?¬npº8T?š•°÷s?͟лN\?²uuë†É"?æÑ$ìh8ã?²ýÛÝö?S?¦ÏSY'1?°>
"Q€¨?©«!l'?ªՕh«(?ìø\Ùy°$?¹C2ËzÑ#3FGL J1857.9+0355@B•Î|Ð57?Õñ÷(ÀéjÀ87¸Óñ"À9Ü7i"ÙI?ûMFˆï@Cˆ?ÿõ?úÆ3
nmò?ïšÞw3#¿á•¿Ù8/¿êºÜÓç.‰¿è"HÒõ UNASNone?d î㏘)?i¸]d*;s?ƖLäø?Ǔ\O%¸?êEÚ½ã2g?ǬåþÈ.•?…c'¶ôÇ?¢zCx-þ?ÅQ]4J³?Âq6×éff?êVj†wJ?Ãsb3ëû?¤¶ð‹‹?"‹Ÿ­³Æ?Î]›÷ÆÈn?²XI—?ç*¥¬?³juÄ2 ?.šöØßÏ?˜¥O²hX?Ъˆ]èEa?Ái™Ís¬?æÁFùUQ?ÁçŒûÌÔÉ3FGL J1857.9+0210@AÍÄupÅ¿ÝyO܌À7iKB±ÂÀ9³ŸAyG?ý­åSViC@dõOÍÈ ?þ=Ž@u"¿äf©#Ǩ¿ã3"]¼¸q¿æ÷ègï
Ñ¿ìÕZ›¾CUNASNone?AÑ'ۄ€†?<A-VÙ-î?â8˜ñ|š?ÐÉ­m,?Ûò¦:/DŒ?Ð܈V1`?A__Í­?aΙ;(ø?ßZ½¦	?ÅËlY\?àzúßY9?ÅÓ§t
'²?"¥Ýª¨`?‡«.µé•?âo͓Yo?¸®Yò
ãÌ?Ù×t"ž¢Ÿ?¸gIÏ/¡ä?ˆ¾"4@å?‡0µX$R?Ô&2‹'=?¼ÐÂ/U"–?åô]çõÝ?¾‰UÚ;j3FGL J1859.6+0102@AeUÅ.rÚ¿õ¶âdä†'À8
šôãlLÀ9ј:ôÉ?÷i§¡D2à@éüíÑÕ?ÿ'%Ÿ í? I^Ó&¿ãoòÿïíl¿æJÀŒ¼UJ¿îŸØ"UNASNone?tÛ¯¥&Qª?rýžpi?ÎÕA½žÂ?ÈyZ¹uþw?è ø1N+m?È¡°dâ?± VNõ`Ã?»Éœµþ
\?ÒOOýÚ0G?Ç«z»¦?ä´M74;Å?Êâ÷dŸ?¦Ö'I"?™)ҘØh$?ׂ?¤'¡é?·úKhíe?âÞw0"
s?¸•×ê)£s?®M»<!Äö?«(üHV2®?Àt}$Ð;?°™Ž;N?êÇ,ô¯¢?¸°}#y'3FGL J1900.8+0337@BœæB¿˜1¿Û£Òm¾À7°]«¬Á•À9ñïÞIÍ?þ9ì$ÖÏ@›,ªØÜ%@͵^q$…¿ÓfÙJVê¿êt–Ë'–ô¿èèæç]п/âØõUNASNone	?Ru'üؾÎ?R]¿k}}o?᧾y>\?Òö97"?Ýæ:ðª‡?Ò'pê©h?5ýu·
'–?Y'$¡W¨f?äÄ+nðP!?Ç;¤³í¿Ë?Ör)ıœ[?Ç>mIï'?¥ô^ÁBÍ?˜xå?°s?ÚüCWš¤?·I˲…|?á"˜'@A?¸
xˆ,ù?'/8ìÅÁe?|ÉB[iÍ?ÞÏ)hoƒ?À'ÂxÊR?àO®M˜±9?À¯çwðîq3FGL J1901.1+0728@DXÁTɅð?óþäǕUgÀ8.üóEºÀ:8*ù?ù霾è¼@
Óô²š@}…¬o	¿äen¿æ›Ž^RÕ¿çnÿ¿Ø¿évPŽã³UNASNone
?'žbZÉaÛ?…FK&óÄ-?ÂE¤¸ŠsË?ëäÍÆ?ë$Hr=…?Þ!›fŒ7?Á'¿>É?Å8¬Ì"ò?ÈeeÕY¥?ÂC8€Nm?圶º÷Uµ?ɾe'|K?¸µr¢Ôí?£n4 Ä?ѵigÅ}^?´"™žé?ä	Hæ´?¶N[#»›?±fÉA"?«ۃñ¢ ?Æ*ämUò~?¸z¯l·ÔE?èH"Kz›.?½+"L\3FGL J1906.6+0720@D˜±_ˆü"¿œ6‡P–ÆVÀ7îü¢}nÀ9áa£‰¤@'a–óÍ@
ØK)tª?ü¢üSøû¿ØŸtùÀå}¿âhÃQ46O¿ãî¯=B¿ê"G§"]UNASNone?GӀݨ¯{?JYnȔ?ÒõO‡Ø?Ìÿ¶|"z?æc[܌T?Í'tƒ~…?$'bqD.ƒ?RPõ"èf™?ãtÈõE´?Éø"v‹Ù–?ÙÛé'¤?ÉúGÔyuì?'&¢•Ýj?‡?íÕ\Õ?Ü.¸³W¨ã?¿~"Ú,?áWn'¥Bº?¾ë殖Ǒ?oԝqÚ=?j¿†!qÞ?âks6P?À´…?Úép¥ÿ‹ª?À•Ÿ]n½3FGL J1915.2+0954@F9q!«K¿æ'"€zä£À824Òo£ýÀ:3î*ëf?úL0':+ @TYsŽÃ@Ú1'w¿ÕZ8äD…¿êÀ>/ÕI¿çÙŒ/n¿åó¡:!ä×UNASNone	?ƒŠÿ®œ?"DæϘeì?Å´È%Pi?Çr²EÓÆ?êD¥°­+?ÇÁZ÷#~?"RΘRÊÒ?¦•a¢²1?Ìe¼†¶Ïþ?ǪN??èKúiµ«?È#UcKò¨?µ"ƒj›ÏY?¡S`²:2ƒ?ÍéD	hÞ¶?³¤º'þR¨?åՐRNg?µbµbé]•?¶ÒZáÝ??«› k}?Å=ÂI'ì¿?»–‡E2¼?çÖDzÉ(?¼Õô6>s3FGL J1919.9+1407@HZåÿ£¹®?Îó_ތè±À7Ȓ¡WÓüÀ9õ¦gÞ5«?ö{ëV¦@ܲ_Ž0@|®fÛ+_¿Ýº}ºjõl¿èR	c¥¨¿èqþÂé<¿æNkwQUNASNone?€pÕ×F?'Š´7«ó?¢9/þ"ú?¬'^+¤šr?¨¹§°?®x¯Tƒüe?¡gê`´×?œ)ìèÍ?«üßAíÝ?¦S­ÈèGÕ?íɬl7¬ß?­H\Yù¼?´–•u
F¹?¢ÈTmz·?Çi¬µ"Cq?±¸k SVö?ç'Â#ùFM?´\&BØü@?»˜ûp&GH?°ç9^õ|ü?²TS¡ì?¦	h¹i:"?êBV1Z"Ù?´y(aÝî3FGL J1921.2+1506@HÝø>Ÿ?Ûi' hÀ86uT?ó5À:V‹"ÞQ?ÿ̒_"Žh@ƒjY5@´s0T¿Ä7·sÁ%¿ë§äO‡¿î•Uël¿îfžšŠZaUNASNone?€"ue‡k—?¤Cr°>
ý?Ø$\¸¦¢-?ÑïK`gŽa?ã«Î';?ÒˆŠ¨+Õ?V(»iÕ?"ÚFlS?ã{ôFw@?É?ڀ+w^?Øñî·¨~ù?ÉR§'à)w?ª®eÉ~(M?¡%³ùø?ڟ6E•g%?¹W"KšK?á~€iè?»,ild›2?"gñO;??~ðHáU¿?æ[¾ÕK-ß?À©""ê?Ò¥BÊïË^?À[ªp$3FGL J1925.4+1727@J%]Äuq?äp?ÎL(ÍÀ8•+á/ZÀ:`Þ	53?ýj0'|G@Ûtä®jâ?ð¡ç¹b6׿Õ9n€ç-¿Õêߑt|¿ëÉ7»qõU¿ïÿâ–b­tUNASNone?RÀ"ëj5?YŽgÉà-?âÓ>XZô?ÒOí]×áÑ?ÚG¼Â»^®?ÒPÏaAõ?c‰Ô¿™ÿé?"÷n0Æt\?Þͧå²l9?ÐaúZ®?à…¢8g/â?Ðr9Ǝ?›ÁÓ>x¿?'œ€Õ	|Û?äénïü?µ–êˆk§o?Ôq¿î@Ò}?´ŽyŠwî9?'ŽÄ|{Hd?'(JV™gl?å›z²…`?Ƈ—Eœ?Ó S-‹P?Æpm[+3FGL J1928.9+1739@Jm[[Õ?}&3ò"'À8imOŽ³À:4››ÒXþ?ú@ÈÍcˁ@òlÃ!Ó9?úgRژgj¿á1ç)€"¿åQƒ8aÎÛ¿åÇ[sÄ¿íµ²ÔÔUNASNone?Mˆ*ÿð?OÇZ‰r?¸©¾a~i#?½·æÕÖõÀ?ìãƒÑÅs?½ÍŒÐ|-ö?Z¢ìÁ)6?t"$T þ¯?ÌU=>9?úuXE;?èò£_:'?Ã5/p-X?¬)»Û‹?š&O½íÊ?بi¯Ö[á?¹p³ðÆox?áé:lW 6?¹'JýP£9?©åIì?¥M,<~j?ϱA‡Ê·*?¾ÑE:‡Zö?æu[
-u?Á"'ÔH·3FGL J1946.4-5403@u~6z—À=ûH
[À94ìð{(À;µû-2h2?þρËDz@
r©rՊŒ?ø·÷'¿7?×¼ê×yÏ¿à܍¸'¿è½ãJ' V¿ìýco³c'UNASNone?je2´)B?p7»'F?êA·=Ði?È
(±ô?ÇMdX8D?Çß°ýGØï?'¸¸*³?'õÃÂÐS?ìoo¤þ?¹ÝT±ù?º-pBzu??·ÁâéȂ?¢Š¿B'?"c¹Éñ¿Ò?ëô[•î?©1Ý9Yt‡?º»R%ë4?¥þê1S?šOorTÖ?:ü9¸$ó?íXā3·¦?¥ÓúmØ>\?­L3š ?££S'µ½É3FGL J1949.3+2433@NšiƒQY¿çCM\ª%À8ÍSù|X@À:¬°',ãŽ?ùƾ•|@
ï/"Ã?øâÞ0¿Åçö-z¿çnKŒ	Qý¿èJ6F°_ü¿ïýÌø$ÙUNASNone
?dC'ïù?ö?m·
`Þ¢ö?¸¹µ'Õ?Ágš$DÇ?ìéeF`e?Á'"Ô_*?2ÈÁBsFú?_N@¼½ûÔ?Úю|õ6ü?Ì¡µ•Løæ?â"ß©]?̧t×®.O?¶Õ,…_IV?¤éí…Á±?×ì&·7µ?¶Ó(©Å:]?á/GÑúú?º¬rs›š?£l˜ÓYÝf?–·´Ž¾?áV÷Ê3S?ÁÚž?Ã?Úæjö]­?Â-ß­P
³3FGL J2017.9+3627@R¢ª:э&?ÚIECVÀ7tUóQ›ÔÀ:1GNs*š@A(¯ ¿h@
{œüOœJ?ö"|ôÈ>s?áô3ˆî{ž¿ßå: &)ú¿è§°[…•^¿ïh]QóEeUNASNone?µäEÈû?ü^ä!´Ù?頚->ݤ?Ç
ŠRÇÎ?É|ìÀ0v?Ç
UÊ´?j̹X>?8 sµ9Ió?ëØÇN¼ï‡?ÁB'€I?Àš÷²ª¹?ÁBZÇ"á?qà_œÙ
?pí÷ÈÓ
?ë¸'ñ&õ?©Žv.Ÿ?À]=;e?¨È|Àñ–M?B…C¸
´¢?AäZÁyM?íoD©+ü?§Ê¯øfg5?³ß{SFŠ¼?§µ6t2%&3FGL J2023.5+4126@SÐ:>À/0@»|,ÑðÀ8"Ð=1À:pñÒ?ÓU@hòbˆ‹@ ŠÒ+†l@BMec‡¿Ü:&ôØÑà¿æW?ÁQ!¿î^måû`οأ>ÍUNASNone
?Êåëø§®?Ì!ãðž@ä?ÜSŒèss?ÑH5I:Ï?Ö9ûvÄ6?ύnü|«.?о.Òår!?ьB"ƒo"?Í+ö"õ
ª?Ê÷»&g˜L?àUêñPF?Ð>0·§&Ù?ÊS`¸¼Ýé?±Ðeµç™?Ó NáêŒ?¶Ú<§¤_@?ßµÂT¿¦?·ü!ÿò¦?¯»³5‡ù'?«©Mud²?ÜHèÖÁÏ?ÑïLfMC ?ßø@°x??ÐM9_F
{3FGL J2024.6+3747@Säy'¼?°«'¡Æ3À8¢×áÓÅÀ:vXò	8?ú*W‡PkÓ@MjàɃí?ý©£A«q?ƒÆó¿ë ǾΏù¿á8ÌÈ5‹¿êú¿»ä"ŒUNASNone?"[Ú$Ck"?Š'®úMßÂ?¡w!¢˜?©•|v?îI%œØ(?¬¤ùj?b¡!¯"j?,Õjd?i?¾r)ŽÆå?¸)1¸™§?ì*™"?¸¶…[W?´èHõ?¢Ã÷a¿.?Ñ6¯~,Ã?²ºOD?äÇí	žg›?´ò7ñ0U(?»y­ÕóE?«—"¨q?Å*U¶ú•ì?·\«ÎWL?çF4ׂø?º•hôƓ~3FGL J2026.8+4003@SŸ}€^_1?ðf¬ƒ§ÀÀ85>˜ÂEÀ:S½ei?ýöâõÙ@ð}0Ò?þ̌ÐÞT_?î´®>R‡H¿ê³¯J¤Ð¿èÏÀG¶Öt¿æQA~6UNASNone?´Ë5¶<ÌJ?¶Ò}ñ²j%?Áš-@?ÅÊgI?éB­o?ɕòñÀ‰?¢ŒV<ø"?¶ã2?Ë¿É³ì`?Çè
ç"Hš?ççW)Ò^?Ê)ë݊D(?¼@ð¦'Ò?§®»ódfc?̬ï@eÏ?±¦k8Ï΀?åL¦:"2?´îK9Ë^n?§)$á:¨?ø±J†?ÓïoáY»¯?Å?]ˆ~$?䕵ÁAÎ~?ÄÖïÇìà3FGL J2026.8+2813@Q5éÍ³}ÀK5°»õÀ9˜d
ƒ À;:†œfÓt?õà—Ê·sÊ@ᓿºëy?ùj§ŽN⼿â2kü¿Òs=idj¿ï†)ñk¿ïýGwtUNASNone?·§†b—°®?Å3ÕøŠ÷?én94Ž.ç?ÊJb{=…¸?¼æ¯øöØ?Á wM™(D?‰IϽ|œ?Ÿî2ôG?çĤ^x?ÆVfã­Óè?Ñ(9å^¤?ŘÑ`Ë	ß?È=³NŸ%;?¬åp‡Þxª?㐬Ô_'ü?µ8Xæuñv?É™_ä:Õ?¯ùâúøìØ?§¥ê¥á? ÉiŽ?lb?ë+Xίt?º'ýäG?»g`?µhú_N3FGL J2032.5+4032@SàÞ~¥øM?Ü
#$G]À7 dJ,süÀ:*†ƒ<`@÷øµ"@;U«3@˜­×êN¿Û‰å—=¿èÒ~?ԉã¿ïÿÌÔY‰?ïÜn~Éð¶UNASNone?çè¦b¯Š?Ñå!õ[H?¦‡»]˜Åw?¹¦Û­Ä?Ê»wÝw?ЛKßu?ÙÙa"ÔZ0?Ø+¼5‡F?–V+oW$µ?§'×àÃBL?â`âÃ?×ØN©
n?Ճ,«¶?¶ØºŒð9_?ÈægÒÄZe?²×­T
x?Þ	Ÿ–òÀ?º1eÂVT ?êVvj¡sÍ?Å´ãô´\?ŒA¹"{?§é–êéÌ?Äâ
āé?Å(Ò氆œ3FGL J2032.5+3921@S¤´·,Q˜¿Ñ0l娶À8,Áúá³À:T
ހS?þ/}Ç/%@3'W°ëñ?ûÛ@bƞµ?ՇW€M÷¿ä¥fÁÕøÅ¿ê`*èêmO¿çºº•VƒUNASNone?JÙ9#ë}?¢n4Ék›ï?ÓÀ¡ô«ã?Ï8ëÇӛÅ?å5X<4
²?ÏÝТ9?SþDOø¸)?j?àÊ)'â?Ðÿ&2ÛAð?Æ»ó8¸"í?çvmÄjb¬?ÆÆu(}€ß?³*~ߌŒ?¡o)œ¸È?Ñ|0ðjæ??³ÑnQ.ip?äܗÅn›N?µMjïäÐþ?é¾	ÏR?"qË©ê†?Ý¥P˜I»g?Ş#ÅEa1?à>	ÃJÓÒ?ÅtIºLk3FGL J2034.4+3833c@SŠOv_Ù¿ð®â5ꝘÀ8^ìÔªÀ:‰Ë—B§D?ú&ñ–…½ð@›àÆ©È@;¢F¨0¿×¯‰Uw¿ë
¬ÑÚ¨®¿ë †?A*忁
cgÞ>UNASNone4?»N£€äà…?·™b¸Ÿ?ÛÏ]²ò–Z?ÐC/MÈw"?Ý\ùlÔ1…?Ð<‡_ñ"ƒ?Á·"Ã8(?ÉÆ3Ž!¯«?½þ
Y
–>?Ä)I~ªóÒ?çÒ}Ïí.?ÏMûn7<I?È]- °?°ìç
†ý?Íï'›Óþ?±¾Ç¥»N?â}/ÑÔ?·õÞÚ_B?عæñäRy?ÆTKEøP<?¶`&Jƒâü?Á'Ñ1³h?à×½½Zd?ÇÌQÝìN²3FGL J2034.6+4302@Tq?l&š?ù¨·^¦~"À88;·f3À:bþ;â?ÿaºÅc@
ÉY;°…C?ÿ¾–EÒB¿ãRêCçG¿ã¤Š÷t¿ëpK&L£¿èáX'€_PUNASNone?x"6'û(î?ó%eaÛ?Ü`8Cfž?ÑëÔ­jˆ?៟qrV_?Ñúšc'?—–v÷?©
ù˜)áv?à—Ì9ÓØ?Ëæ7§o¦?Ý^ï'ðàY?Ë~ø|¡Í?Â'T§^V?ª¸ã¨|?×ê
µèÚ?·*Ó4jSI?ßáŸÃv½?·K§WK?—`åxS†5?'qFØ¢?ãÎÖ&ö'd?ĊŒªÀV@?ÖìEZ¤Ó?øͭ1Ö3FGL J2035.0+3634@S(ˆ&ªŽ´À†»øiÀ9°à<4À;
-åìY?ü«äåS@²ìì§Þ?ÑNÓã:?ïêÖò"[3?™é¢à.Y¿Ö¡CU®÷é¿ï0#ëËUNASNone?ƒ¢±L3?¡"ÒuD?è–íù(ü?Ðs"ö{˜?Ìj':äGN?Ð<º§ÏiÌ?'½R¼Œ?¦^t"|Û,?àÙ´d?ÒñÅu‡Áö?ß@bémS?Ó"®Jü?¶$ӝj'?£»_2å]¤?ç¯-O	?²jt·¨?Æ1‰|3ò'?¯s5ÅÀ?ÀŽY1'/"?·s@Ï?âáʸ¬?²?ÉׇU(?Ñõ=õæhÑ?ÆÚÊA³#³3FGL J2038.4+4212@TaÄØì–?á]iR‹¾À7ö;¤ñ¼pÀ:ûwÛð?ÿSÊ7F=Q@'<§P;'?ýC7àlõ¿¶ÕA™(¿åæà/'N¿ç°—já¿é8‹ÛÀÛUNASNone?Ywêù0‡?Z™²þ.l"?¶"!:Tߪ?ºwJ‰âáŽ?í"¿ã8›ó?ººwA?yNÈÚÚȾ?9:ø"V?ØOßnó¥¤?ÉDЪí?ã¥r¶Ðwœ?ɖnh E?©L?D*L'?˜ÏÝèÿ??ÑAÊ‹ù*?³¥NÉÓ·€?åÊVü÷^¢?´>¨mžõ`?—ÁÉäwV?'É|ûñF?×~™Q˜?Á	ˆ ;?ã²2¯žr?Á/†2®i3FGL J2039.4+4111@T5¨mqó¿Ê'¼£nÀ8û'²õ‹À:AàLÜQ¥?þìñÓA†@…̘Ih@ê:Ì.Â5¿×´È\ƒAF¿èPÎáÇR1¿ë58~v¨~¿äÝaeÎUNASNone?f2Ý	³˜?jÀëU"¨?ÀŽ<¢)?Ä"E•Å?ëÆS¤œ?Ä6ìÏ<è?lÖ7÷¿ð?‡œ;L[?ÐÝ
ãð"?Ç7Ò~BVA?çt¢þÏ÷3?Çt¨G§NÆ?³©¿'%?¡†§}Uc?Еbþ9"?¸½N?Ü?£?å@Bn0Ÿ'?¸ýÔ껸(?£/(Cp6ƒ?›¹ªC?ؕŽªQ+?ÈKÿ0ü{?â'´sÔ?Ç2"ɉñ3FGL J2039.6-5618@uS²þÅm]ÀB"Ùý6÷äÀ8ʇkŸ‹À;O3·½q?úfý4Ñ@Y…kE-?û-x¦¯×Ÿ¿ÑӂMø†d¿ÝÝ'ãɾz¿ãˆã˜/% ¿í×)5óUNASNone?síàüïv?Š?h¼Á?ë&ü±š>Ð?ÃáO˜S¥H?ÁŒÎ[‡5Ë?Ãæ¨ËMÑ?Ž4CíÕå¼?—ŽU2¤¸?ê"K¼Å‹?Äm»SÀvb?Å®ª'/‹w?Ã:±khzü?¨±K&æ?–j–M»L?êP£ø§?­¡,'Odì?À'_Kª
?©Už"'U?¡ÍKdhun?'؈ð'Þ?騞?f&b?³d˜"Gh?Äê4)MI?±¨K;êÓ3FGL J2041.1+4736@U…Ó™o¨/@±€%TM_À8+Yª–AÀ:ÇvË8x?ûöžšŠZa@…4"@ÔŸgd¿×bYäfü¿äÒø/§Ÿ¿éN9¥Ni׿ê(±Žû'vUNASNone?¯Áï^×{9?¦sÊ=ÓQ?ῗ˜(P­?ÌPz³`¹?؈'ãÔo>?ËXŽ×|›j?¥ö$cOe?°;H֏Vo?Þhs? )3?ÊÂ<Áˬ—?ÞØÈ4uê)?ʘ 	¾?ʀø€«–?±g†]Ŝ?ÚÔanØÄ?·¶wßÏru?×ë"PÒq?·jm6‡?±<r}þÅ?š´ƒw·)
?äA{nÀ´	?¸fE9h{?Ó.Eß;?µueCþc=3FGL J2042.4+4209@T{ªOÊB¯¿²;X6LîÀ86‹ò)ôÀ:UÊ! áø?ú)Œì7 S@GØ4ß۝?þíâ¦Ó¾Ù¿Û¦IŽ‹Á¿èq®0Ý÷¿ã¡ÄZ"Ó0¿éãP÷,rUNASNone?œêc9"?'S¢ô H?«åòß)æ=?³5›œÖ<‡?íË-)ëÔ¶?µ7ÙbL8?bŒ8PA Ú?|WÆ:s½¬?Å_ü¹¥éš?ÀKóÛ)?ê•t™FCù?ÀUÃÇ?¹a»¢`?¤«—=?Ë$ãbÊ}‰?¯Ç#Aî§`?æ
¦¯ìŒR?²ånþ—™?¶Jü‹¤o?¨·#g"ð?ÉA4%#µÄ?¸D'ÏÃ"?ææSeB"ž?»àªë43FGL J2043.1+4350@TÕßeUÅ?ëﵩ-‹À8"Íui8©À:· ×æÜC?ùƔ·1¯û@wOz;°Z@ªWk÷ ¿Ü7âȕ8?¿í§"€"¿Ø–§XÁYž¿î"i$ösSUNASNone?¤yãĬ?¬‡å=G:m?Мñ³¾M‹?ʬ*ÿ…ôº?æp•Rœð?ÌòÿKñK?‹àpú?£ù:±\A?ԚàMSÀö?È}ld/èè?åF-ÑÕÑÂ?ÈÆ£aû†*?ÃWÖÒÆý?ªŸC9f
/?؃ßî–Òü?µ<ü~?ÝÐ5Ʌ?¸…õi?ñH?ÂöÔ^w±?±£ ²FzŸ?ÑrG>:Þè?ÄIÝçaÑU?â‰'`Êò ?ú~Áb3FGL J2048.8+4436@U%+ÓÃa?át0‰4LjÀ8|@lÚÀ:à&¶ÁÉ@!­ÎYê­@"R£eö)?üîԞþ2u?Ç`MŸ½l¿çôò"䣿첻尿ïÿ" ¿mUNASNone?Æa'< «9?ÂTx=#Ô?×v˜¡fn$?ÍÄGöÒ¶ª?ÝXÓÀI<??ÎèÎUƚ?BX¡»œ?[0ÎÛsÆ?࿛a?¬¼?ÌS‰:Ug?Þwœì¢æ¸?ÌWù""I«?ÈÛ­^«œ?°uÒҗñ?ÝçàÍaH?µ­2ÔÅ?ÕªIXHé?µr¤ :`?'´MÓGò?…'·ÕkðÚ?ë(*?¶'ӻΆ?Á˜Õõ|.œ?´¾§kwÀ3FGL J2103.7-1113@BíÐ|"µÝÀA6)Çy¦µÀ9Í#¯1±À;¿VŸI?÷9`üÅ
@N¸Ê·H×?ñЉB37?ïÿxùsŸ¿×¨ùD5J¿â7îÕú⤿ì
Bùú­UNASNone?ÉFÓ'
?Ä­±`Sy'?æìuùËÍã?ÊþÔaÀ·/?¶ #ûBÑ?¾¾B÷o?ÔãF"©‡Õ?ÊG¹š®?Ú¸&Šw?Ìuãÿ>æ?Ðd'áCi³?Á±ôÞ(ñM?ÅÛ³Ü.Ö[?±ßf®-?æŽÊHƒym?µi¯Éˆä?¿ÒF†‡ß?§Š˜±µ?ÚQÝõ0î?¿øSC×F?ٛ3¬:¨E?¿ra%YK?È%ܽ(Óf?ºw°'Y¦&3FGL J2112.5-3044@-Ì`RP/ÀE9nÀY!À8¯¨tþ¯žÀ;N%@+i:@ABŽ@•ä¯—‡Ç?ñĐ£PҀ¿ºTqu§æ¨¿ÐSF"ã!M¿áG¡>Ô|¿ïÿù_|è3UNASNone?©0}\†-ð?¶ìI	QK?ëý6…‡?ÆY(ÑÄ6?³~í"ÌÕ?ÀluÁ‡Ìý?'ˆ|µ­kˆ?Ÿœ«›€ƒn?ê&Ê>ûÀ9?ÆKÔ!2§Å?Å3Çm[Qª?Ä|"Ç|£Â?§;±açL?›R'7,²?ë"Äéƨ¥?«ƒFŽ>?»L×Ð?§•žU/?¦`‡A*?œC/í[í?ê1xàž?¹<,<N²å?Á¢ú»÷s?µð'òêq°3FGL J2114.0+5239@WWn.±Ä3@ßT•Ð·À9,Òn¥ÐÀ;ÚPp[?öaÅõæ@)0¬›)?ô"rþ¥7?ïþ,0Á®¿çX/ŽZn¿ê\¼:û¡¿Ù­k+$ÏvUNASNone?Û¥ÚvMa™?ÐCµÃö[I?ªbc-:i?°'J,¬Pà?à†ì'¨¤?Ñ={}÷˜?Þf#ëô,?ÕÆG{R@Û?¨»9¨'CS?±/¢`â?ނu¿Ãi?Ô¯N°!"?âÆ&³úö?´%u,K˜ü?ÆK'—5žq?ªÓ›~"D?Λ✊u¹?±³ü…¾?àª-Xóm?ÄîÄ4UË?»Æ\u¡×ß?»-µØ=?׉‡å£.?Å놀ȂŒ3FGL J2117.6+3725@T³ {5+À Œ$=Ìê)À9´ã¡ûhÀ;[«Åìû?÷º¢˜›Â¿@ImÖr=	?ÿÚ.ÌHî¿Å~Þ]ÕŽ¿å))'¿éˆWHÕö†¿ïÿÃ	ÌUNASNone?Ïz`•!çí?Ä<
Üäs?Þ…Ö¹!?Ëpè?Í?ÒAJš˜Ré?ÅØòZ»>2?"ë@^sRÂ?àúÁea?å­0ð?Æ´xœ ¼?Ófëø7Ì®?Æ8½Y$¨?ÎñÔ¸¯o?±àÿPæk?â;¯±;¬?´Ù¤"8Ù?Èl'bKq?ª"E¿'®O?¹<kqNÃÓ?ž||ý°ÆÞ?ç÷o7¦	²?²®ãeÅ&L?Ä
hÀwM?¯?÷*Á(Ä3FGL J2125.8+5832@X¯iì,äe@Éú©u°À9'][û©YÀ;ˆ*…È?ö9B×@I@MãÂË ?øÉZí6yº?ÒÀÖc=Uæ¿çmõ*ÜD¿ë:¿»Óg¿ê¨»VO9UNASNone	?ÖrÈò‰¥ƒ?ʽÎeòb?ÇýKª]{Ý?Ã1'Ïå³?ݎ'8Gœ?ÏÆ¡mf?Ö	c?οw ?ËqÊñ­‡?ÃÉ81g?ÜG$&9Z?Íf"ìS¡"?Ü(çߐ"'?¶1Î2ĸ?×FœÚU"^?³Õ`Gýø?É öŒ5v!?¬Þ©‰¡y"?Úþód	?»÷¡dÙpm?Ø9¤uh?ÀȬQ'‰¡?ËL¹/¶ý?½Á9ªNÁ3FGL J2133.0-6433@t‹Ò½<6ÀD¢VÿÁßÀ:@ËLš†À<	—@G?ùþð`z¿@B°'¿7Ž?à~ð~‹Sä¿á'òWBT¿Ã4Ì}‹¿é@¢¶½…¡¿ìiµþK—PUNASNone?ªW 2ü?²ÆžX琗?ê¬_Wœä%?ÊÛ±{Ã%?½ˆÅV?ÆÜկϠß?Ñ÷+ä n?Ðp¥gšDP?Üý¢Z‡þ?Ñm¸ð"p?ÑO¼ÁW–?Æ2ÝxO?ÆšÛœnç?­k– B?ågQÏ8Ÿ?´¡Ûc5°?ÄTçÔ?¯Ræ°¤œÚ?ÚSOœc˜r?Åð"0°?ÞBf¦ÞÞy?Ç~ ªNÉ?½©&òö$V?»§h°e43FGL J2206.5+6451@Z¡ï^Èt@'W«¸€À92FÀ:ü¹kÆøw?üÁ"\Ð@ef»ü@…újꯌ¿Ïøå!µåÞ¿çғâº8º¿êŒœ",r¿ïÿ"Ó¿¸ÆUNASNone?§‰/µs®?§	˜2ù†t?áÏò[–ó?Сµ†ð÷?Ùnõòš\Z?Ðu…NHÃ?^vãL?"ŽníÅ$Á?èÙ¾¯üT?ÅÕþ=Ö¯?Ë iH"W—?Åi2y@|¯?ÊͶ+äñË?¯¾EšH.?ޓƒ'‹e%?¶ ˜µöû?Ô¡Â'!ö?µ^CW¨ ‡?̗:+?ƒ«¯s•L?ë©z9œ×?±šJ'ïsÿ?¾ÑÌ 1þ?°'‡®g¹3FGL J2212.5+0703@Q/‹«`kÀCHP½‡µlÀ9nv½ÌÀ;™FéÉ\Ö?öÙù΍—-@4~…l?ûHÙÉà^¿Ö$;"Ì"¿á*øú¹U¿ä7û"i¿ïÿåFúUNASNone?ÖŀG­?ÇÇL•°e?àV¼J«A?Êꞕq¡È?ÁFç#¥?½Ì ¶ú|?Ò҂	÷{º?ÇUB×Þ%p?Û'ã1;¤?Êùñ*Ë?Òû×H¢?Â¥ÀN}?Ǹ]¶«Ä?²‡ÔÄǁü?åöFHñÃ?µ µ‹è?Àmm0¼/?¦Ê:šíU?Ûî%Èóö?¹(_(pž‰?Øbî´¢~?¼Çãs"ãC?É×]×Ó?´ò	ÅvZë3FGL J2221.6+6507@[¿Ž`€@ÂQã!¢èÀ9gJöžWnÀ;ç½?ùû÷²©‹@M;G(Þ@…xì?Âyð‹1»©¿æb©\h¿ïÝÂ凮¿ïGKI½ÂUNASNone?Òþ>þ?Ë?Ώö ¸?᪞öf)?Ï\¢ÓI¢<?Å-‡¨iÉ?ÃðèŽà±?Åh¶:I0û?ÃgîCN<4?Út4ã´?ʚŽn'™?Ú×oÿ»³d?ʘñóрN?Ò_¹Y9éÙ?²-ãÂÿ(?ߥÜôå}?´F.—k¤/?Í7A"¢aQ?°ZWØúbÞ?¹,qYǟ\?©ñ|ô)p?æ®Î4º.i?ÁïêY[ߤ?È®Ž€3v«?»>""ç¯3FGL J2221.7+6318@ZÁeUÅ.s@›¡±–À9(‡%ùŽÍÀ;&'d@ò?þQH,>¢R@
;ÏWì{?ü2ßã«¿Õ4o)>ÎÙ¿ç¡äÞ³Ìm¿êüÇ`sª"¿ç"îrA™†UNASNone?½ô9Tt\œ?»1 '×6?ٓ¡LO•?Îh m£J?ÞïP^"SL?Ï_ï2Ü?¯6ïæÂÂÉ?¹†á™ªÇ^?Ùyjrε¯?Î9:ç,Ò?áOÛÈ,xü?ÍӇ+øï?ÙLþHZâJ?´ïi˅µ@?Ô8ÊÅk»—?³4'k&ÒÇ?Òz6ò9b?´(ý¥Ø ¬?´ÍWÂð«?®+´è•Ç™?å/^
r?È ûr¶—?Ðmíô"ñ?ÃÓ¯B¹Ÿð3FGL J2233.1+6542@[UîËûµ@>Û<ÒfÀ8ɸKgÝÀ;ØWDŠt?ú³
-ºù;@¯}W´@uàŽ ¿á"ŸÇ±¿æ±.–kfֿ놥¥Z[Û¿îljˊfUNASNone?£J×{1+Š?¡Æ"¼ÄM?é1DòÛ¢B?Ä\AÝ]?Æh6UÅ,?¼»êÿçó?¨¡Ê†l?´–»€½?åGT½À?Ê7¯¯Ñ·L?Ò]3¿.\?ÈÜ'±E¡?ÓØyí0;L?±WYêw&è?Ýä:b–xÌ?´ÁJ
õƒ?̆—`r—Ñ?®;s¶#?«‰d3jø?˜k֗\«?éZŽ›ÉÌ?´Ø]×3Xc?ól"*É?±4õi‰u	3FGL J2237.9+6320@[&E^®â@öj}L[ùÀ9Z¼ËÍÉLÀ;S:ঞ?÷¼©ÑË\@ T´àó@ü«¶Q¶+¿Ë1Š$Z¿¿ìˆÐí*¿äÉiý
¿ì¦
ÆŪLUNASNone?­"fâz…	?ªòV')~Ü?àßîqð7L?Ì>é2øˆ?ڏ–?Ð@Æ?ÌY@s\¯?±ñô4¦"?µ¢=[{?Ù}¡| R?Ȗ^!ñ¨"?áð»?Ó?ÈóƵuuó?Óæéý4A6?±[ÙjӒ?Þð
räÐÈ?²"'³á—P?ÊRÍÜ?ªŸ`ö\'b?É¥–¹ôi?°šÕn ?àº@¤G?ÀÕ>Zªî#?Ó."'ä?¸P»@Ã3FGL J2310.1-0557@Qlvò¥¤jÀLø(¡ß¹9À:b8š{@éÀ<5[½•ø?úØ1rìí@Pž¯®?«ɔ•)?ï¢Z´ñ'º¿©‰ì	!¿åèg™±`¿ïÿyOw6˜UNASNone?×÷Å ''‹?ÔÓ§ž…hü?â ÕŽ<Pc?Ô٭ג=ž?¦4~þeu?ºÜœsMàU?ÎÉõÓЧg?Ðu³6ÁîÂ?âiáVx?Ò-_؇oc?É b¦Õxƒ?ÄÊ$ ä±K?©£^ó›?°°ƒ#§?ç4Gcd?´Õ…gãäÉ?¾+®Vý¬?¨'켇'?مÖÿ|T‡?ɵè^6 ?àÑћx??ÊâCºV¬?¹
u2ëå?º˜›lZó3FGL J2353.3+6639@]M©?)
»@½?é$À9)ölÙG/À;O{ƒ.J?þCaƒ‡4@
J^Èã3?þi™aܔ?ÒéQ؄*¿èñôgN }¿ì€zŸê|Ç¿í›>ŠTWUNASNone	?›€îÄâì?Ÿÿ[òÚEk?å¬ÎF®>?͓`—MÙd?ÒîT'׏T?̖oÚYù?|˵¼°?›ôö_Žƒz?è†vœÂ:Ø?Æ¢CrM'ª?ÌÿÍyf·?ÅËðùÊí?Ì&®¯ØZ
?°hY³1±Ž?áFž#¬?´×
	íw?ÍÔ6×ç??°àº2Tìh?û.ëý¬?"xT˪?ìàê×öYÃ?±§³ö?µ9CbÍ|h?¯XŒ€g.á3FGL J0937.7+5008@dëÿ´€¦@Gbž À:' €©ÌÀ;ömÏç3€À!͋¹‡ @8e>É…@äÀ^g¿â¯îyèÓ¿ç'Ã&l¨¿åîÏÜÕ60¿à¡xhÐAGNfsrq?îhÚú£›j?¸Ý˜®2B?[šõø?hÜßP	¥?¨•Žë3?¸Û}úºk?ï¤è™g£X?§ŸžÃ?r¹<T€1?¡ÀeLç??zҘÙÔ	?—¡ÿw?í¦Ðš–Ó?›on¯vž?™u¤Dt¸?Q¶£"m?¨Ø$4YÄâ?">¯™@–§?ï®Q'Z?¨Z'¢ÏkQ?•æ5»@!?Q´!»5ß?"Nùu3Á¢?¨F>Phô»3FGL J1031.0+7440@`ǗͅY@CšÀ ýÀ:&sÔ
2îÀ;´¦ÏB.À!͋¹‡ @M†ÇÚʑ@,"ß}ÿ_¿ÎY 
ý¿ç¥b•ÿä°¿Ü[z"0t¿äSr€'TAGNbcu?ï4ÐZƒ+?´P(MoE7?cæsÒò?žeß.¸åÓ?–é&= M8?²´ç'ý¬•?³rÆ?¨K&·g%8?rÀÔ_q^f?¡mÙèŒhÐ?v¨ó•Ð±?›úÑh3;?íº¿?ÀJ?š~֝•O"?˜œÍ!%Ø»?Ž	¦yêbË?¨§«q?"Oؽ[Î?ï-³À"ï‰?³+á™"@?·'ۋ?Zm ™!g?š6ÐÎïï?³ (o¢)ù3FGL J1159.6-0723@q'Êßø"¼@J¢€dÀ9Ҙ×ÒºMÀ;¢Òhî#À!͋¹‡ @x†ä'@Ôɀ'±¿æQ:›:G¿Ør‰ñ¹t¿æð±$´|¿¯ƒ-–mžAGNbcu?îj¹ê‰d'?½ÆÜ!rBœ?r'Ö}pÎÔ?ZHK'x±?§‡»?½Æ¯Mû|?﯊­¡Ô?¦iYºNLi?qO$uÅ?¡#¹Ÿ®Ç;?v넺ÛÛ?"²Ø izš?íí5?¢ú÷Cˆ&?¡'D–å"­?'Û[·yÁÅ?®§YÊG)m?œ†ë/4'?瑱!´¶3?¢Ó¦Ý/!>ïϒ1ÐÊ1?0 ÑÆ=Á9?…OîEÿ;?¢Ê-˜Á›~3FGL J1832.4-5659@u#–Óõ¶À4¯ÿ6¬dÀ9>ô×­Ñ_À;–Ë1ÂëÀ!͋¹‡ @´:¹ºKk@'¾Ÿã_¶¿é!á+ ±¿Ù
¨4¼ö¿è­·ŸOLU¿â.e-"ÅIAGNbll?êUñ#ÿ\?Ìè"Å?–#%OU±?¥½ú•úÒ?ÃãÖɹ`X?̬©{Ñ*?ïLLX	}ö?±9"YŸ?o†¸ÖööL?"Š©+6l?'…ãñbƒ?¬D¬§­?êåi›»‹?¦ç¿àOü‡?­yØŖ•%?—xÕ
ðk0?ºËhVÙ?¢Ž"§z?îÉt›Ê?¹ðÕ5ì?:GÄ(E?v.¶Ê‹½¬?£9z­íó??¹®¦ÏPt<3FGL J2358.3-2853@5H€_5ð}ÀSŠ« ,ZÒÀ:GpJ붝À;õxZ"±À!͋¹‡ @žIaÈÈ@OãÀYK÷¿ßÐ¥æ?JÕ¿ê®tŒóe¿ÊTLªË¿ïÿ'£+ÓAGNbcu?îzËìÞ=?¾]h%¼?QÙ£E8ۘ?q#³ù,Ž-?§Ät#èU\?¾
ð?‹^ÝÏ?¦d#ÖM'í?YKž˜šå?|ÎݵcD?‹r³´uxÉ?¤95{'S?ì!¨±ÌÇ6?¢6ÅüBl?«F²#c#?˜Þ˹y³Í?±O¸ˆº?š:²^ôê?溺Âd?µËÙøZ>û%PªýÞ°?A¼f¢ovI?uá¶<óò?µÈ,¸u¡3FGL J0534.5+2201i@g´ßݵÀö@8ªAÀ5¨†¡oPñÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ú=p¡'Øa¿Ó×o9ìh¿Ù3Ší•€l¿ÍÉB˜o¼À¿ÍЁ~+^OTHERPWN?ìɞ/ØZå?Áaô€Qðb?¤‹¶v/.?¶6¹Öû¸Ò?®ÚfŒK#?º§溡¤?'$D^q?»ï^¼oé#?êëc©uL›?юÛCu5¸?Â
îÑ©ÁÆ?Ðg4²£ä?ç­2•V‡?°Ô‹«ËÐ?·ÀPtÊÊ?¥N'sÅ°v?ÇýI
p@}?«ü"wø?̀Óøçòw?ÚÜÜM"Ys?èŸËÆb?ÚÜÜM"Ys9—#9<ÇË9æÚxÃ}Å3FGL J0833.1-4511e@puR}ÔAÀØðߦ™1À6!vu¨"ÉÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@G̀&¿äqªé3q¿æe¥åþ™¿äqªí~óü¿ä§ÍP¢§,OTHERPWN?áª4úx`?ÑÒÍúØuñ?¥ÀŽÌjqú?¶ñjt/I?Ùó"1ð¦?ÑáŒ'«`?"ݤEØÂ?½">Dn ?êë(B¹#?ыoυVE?ÁÒwªl`^?ÐDämà…¨?ã¡_â #¶?°€(
ò´¡?¿›Ì*¼.?¦þ|¾¾N?ÐÖM0ɉ?«wa¥Òàc?͜ڢñ#?ÚéD§âk»?è˜ÉWx÷?ÚéD§âk»9£WØóÐ4Î9óÌ.¦]3FGL J1514.0-5915e@tQ¿zÔ²¿ôWõÀjÀ7Ï{-ÇýÀqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?ù$5½À¿Ñn£ Öå¿×!ƒït~¿Ñn¶t¤J¿Ð…[/aӖOTHERPWN?ìÇӊ9ÑÒ?ÂiAÑbÅ?­"j˜AQ'?½Ïå#ð?¥î\Ä!'O?¶—c'–]?"¯ôû²?½–ýƈ´?êú±¶LW?ÑhÂF›ºÍ?Á'£F°?Ð Z_4?æŸF+‰6?°â0Ô É?·=Î=qµb?¤·OÊèç°?Éä¯È™u?­¸™0)M?ÍÖ¿1?Ú÷;—t;ç?èŠ{3¸?Ú÷;—t;ç9‰C¿-¶Í9س¡£^A3FGL J2021.0+4031e@Sp¿ñ7@'˜à66À92šs´-Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û?øzá? ~æ¿Ð&
ŒT¸¿Õ¨xöræ¿Ð&
±Õ‹É¿¾pç&räOTHERSNR?íÞÐ+\?½c´EN¤?£'ÿÏ~˜Ã?µ^1mŸ¹z?íæ[¡ã?²Êcõ'óŠ?"'wŒ¯³?¼r§y"H?ë!ïØòô?Ñä9g§÷?ÁñªžIÍ?Ϙ}4u¦š?鐯NڅE?­ms£P"1?¸6_ò;MØ?¨"²>Q™Ý?»D%–ðˆ?£˜¥­e,?ÎÏØ%Ë'?Û
23Ïjº?è}	ö6?Û
23Ïj»9†÷'qr:Õ9Ö¯[=Ás3FGL J2028.6+4110e@Sæy€žQ?öVŽà3·À5$‹
Š}Àqə™™™šÀ!͋¹‡ ?æ.Bÿ6´û@ff_°iÀ¿á¸•Ý0r¿ãêáF›3¼¿Ê²ôQ©ž}¿ãÊ­" ®¡OTHERSFR?ã0οs¶?Ñù	ÈÄc%?žáØâč?´³–Lkêe?×±¦ârìL?ÑǬd_?"xx.ó´?½TÄÀ횗?ëÙS*ÏV?Ñ'õn'D?ÁˤNä-?ϲ®øé?å8}/?±#µNyÇ­?¸B¿¤Ð›|?¤MíÄ-È?Îþ~7Vö;?­íc!Åa?̈́#4[,ö?ÚãCKl_y?èž÷2é4Ã?ÚãCKl_z9™I1Ձ"ž9èù°Å-3FGL J1513.9-5908@t#àz(»¿ò—™:À7Ó%ô†O:À9ø˜˜—;À!͋¹‡ @d<˜â'@óƒÀig"¿ìÆ¿u)¿ìž=e^¿áÃn/Ĥñ¿ÒºTûPSRPSR?µ°ô`²µ'?ÂÀXd0¡ý?¨€Yä"Á?½uFG€ÝË?ëÁá>Ka?ÊîýãµÜ"?èSR¨ïê?ÖSí` @?‡Ê`Iu&(?¦¼šÞV¾?Í6W¬}ñ?՟þÍg?Áц0è"?©Ã-ÅÑg?ʚúíP?±öJP6³}?ääßø¸qÕ?´}¤÷ª™?íÁI´P%?Â,OGyží>ÆÜæe4>±ý£ÄuK?±õµÕï°u?Â,Mí·nÛ3FGL J0121.8-3917@qU{à~íÀSË¿ñò÷À:¾8äMÀ;ÿÍ2MZ&À!͋¹‡ @èw9@?üÊb&%Ú?ïôöŽ®¿á°ãôAí¿âO²vE'¿ã2ã#žUNASNone?ïÈ`¿·®s?¨ê$sÜ?`HÁ›u<A?¤Ü4÷¹q?s«?Vn({?˜læ"<ô?臨ôf]?šÍaÔä2?U=´ŽÅØ?xýš€Ký?ƒj¢æÐ?–漙N-?íYwÀI?™'B÷ofR?ž©Imä?º½Ëfë?«ÞÙ:_D{?"ýÈ®à'?ï&ùAx%?´%FôßH¹>кç×ýÅû?}üÊR?›Ì"}Ün?´$È´‰ð3FGL J1655.1-3954@u',à2Û@ÿ8x[0À:fÿš6À;â1¸ß°À!͋¹‡ @;,‡óSõ?úàåáâ"?ìºvçpš¥¿çIÕ·¿ÔuÌX2¿ã'?™UNASNone?ìíØ9»g?Æá"×-?ZõôYÖcu?p+Ì9@Ô7?¸%f`½m™?Æêü^þ?àî`žîÁ?Ú§­µ¢çP?"dlxÓp?¬74Mt?ÜݖwAåH?ÚÆ–|&?çI½ƒèU#?¶±î»w/?¬"tHãÉ? ò¯Üì·?˳ìèŒrƒ?´¿6ï¿8ù?êЫ ˆ'Á?ÏvGAþ?ÿ;ʂ?TKê4éF?Ä»Rûž
…?Ïs×?ß0"

==> SOM_VIZIER/4FGL-DR2_Candidates_OTHER_3classes <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  163 / width of table in bytes                        NAXIS2  =                   30 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   15 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\4FGL-DR2_Candidates...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'GLON    '           / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ASSOC_FGL'          / label for column 4                             TFORM4  = '18A     '           / format for column 4                            TTYPE5  = 'Category_Prob_4FGL' / label for column 5                             TFORM5  = '5A      '           / format for column 5                            TTYPE6  = 'Flags_4FGL'         / label for column 6                             TFORM6  = 'I       '           / format for column 6                            TTYPE7  = 'OTHER_TOTAL'        / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'OTHER_TOTAL_STD'    / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'Category_Prob_3FGL' / label for column 9                             TFORM9  = '5A      '           / format for column 9                            TTYPE10 = 'RAJ2000 '           / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'DEJ2000 '           / label for column 11                            TFORM11 = 'E       '           / format for column 11                           TTYPE12 = 'main_id '           / label for column 12                            TFORM12 = '34A     '           / format for column 12                           TTYPE13 = 'main_type'          / label for column 13                            TFORM13 = '16A     '           / format for column 13                           TTYPE14 = 'other_types'        / label for column 14                            TFORM14 = '13A     '           / format for column 14                           TTYPE15 = 'angDist '           / label for column 15                            TFORM15 = 'D       '           / format for column 15                           DATE-HDU= '2022-01-29T22:25:17' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             4FGL J1800.2-2403c@m=…œŒ"¿Õ¾¤žv1FGL J1800.5-2359cOTHER0@òY
\J?Œ¡ûXì@pàú¬Ùè>ÁÀ†Ž4FGL J1800.2-2403cUnknown?¤¦C̪ï4FGL J1417.7-6057@s""M;?ÆÊ#åbÿOTHER@¿…-{ä(?Ãü›ÐÈ{²@jÎ^5?|îÂsӏ4FGL J1417.7-6057gammagam?'g@€ù£4FGL J1847.7-0125@?<¿\¢˜?ła€"¥OTHER@·=|ÀÎp?Ãùÿ¡ç7@qžýó¶E¢¿·;dSSTOERC G031.2256+00.1711Candidate_YSOIR |Y*?@EÕã}é9ë4FGL J1838.7-0601@:!ç¸
é?°uÙöÖáyOTHER@}(7ñLÎ?ÄdJ%ò'û@q{
=p£×ÀÀ›¦Cl* Stephenson    2    DFK      71Star*iC|*  |IR@7¸Ϧœ4FGL J1838.4-0630c@9¦'"šVX¿¶5U"…XOTHER8@FX^ïWD?Åc¥ÂÚ®@qy¤?åÉÀЇý4FGL J1838.4-0630cUnknown?CUGZ1¤¾4FGL J1843.7-0326@<þŒ&?¹hšY³3FGL J1843.7-0322OTHER@B~Þ5?ÆCKœ&$ßMIXED@qŽç¯·éÀ[÷Ï3FGL J1843.7-0322gammagam?‰ßÚƊ"l4FGL J1556.8-5242c@tŽæ[ê¢?áG›*½™OTHER=@ï¾»?Â0IÌMÕ@m旍Oß;ÂR×Ü2MASS J15564953-5241450Candidate_YSOY*?|IR |*@Jæ"-Qqã4FGL J1631.7-4826c@tþ5'Ì÷¿ÇYϪ!Ò
3FGL J1632.4-4820OTHER$@ãšñ2‡¼?؁Ž§º˜OTHER@nþ4êKÂA¿}SDC G335.894-0.184DkNebDNe|DNe@8FĤ	_$4FGL J1626.0-4917c@têû¨'k¿¶aTâ3FGL J1626.2-4911OTHER<@׫LƒU?ÅÅ*PE£OTHER@nÐCþ\'ÑÂE"œ4FGL J1626.0-4917cBLLacgam|BLL?{U%ÌBcR4FGL J1419.2-6029@s˜­BÃÉï?áöAÛl¢ÁOTHER@Ö6­Ù?Çu$°	Xb@jÙß;dZÂqô×4FGL J1419.2-6029gammagam?z5Ö{¢7Î4FGL J1849.4-0117@?Œ¶0©¿Â¨†z'3FGL J1849.5-0124cOTHER@ÐËúóY\?È8'ÕÝú­MIXED@q¥¹#¢œx¿¦B[SSTOERC G031.5367-00.1555Candidate_YSOIR |Y*?@I–È´9X4FGL J1109.4-6115e@r/Á [À¿èÑØ8så3FGL J1111.9-6038OTHER@ЋÙ¸î?ÌÛÖO9¯ðMIXED@d땁$ÝÂu	7FGES J1109.4-6115gammagam?q°hjM4FGL J1850.2-0201@>ÿ
gb¿åg|`£®ÆOTHER@³¸¶%§–?ʨN÷þ¢@q©+ÓÃaÀ¥4FGL J1850.2-0201gammagam?¥Qï¶Ü 4FGL J1619.4-5106c@tÉoiDg8¿ã°™?׆dOTHER$@®Iݪѷ?ÊN2·>@n›H˒:ÂLfé4FGL J1619.4-5106gammagam?z'^	4FGL J1620.8-5035c@tÑÒò䏿ڦlü,¶ÂOTHER4@)"+¤&?Èʈ\jÂï@n§µsê³ÂJ\Æ4FGL J1620.8-5035gammagam?ˆŠÑ ¤4FGL J1801.8-2358@m\`S&ï¿ãŠoŊ¹,OTHER@›'îƒR?Æo6_P§Ä@pçE¡ÊÀƒÁ¿Ü'4FGL J1801.8-2358gammagam?w–¿Ê…Ê°4FGL J1511.2-5803@t	#c²W¿¯ù ?{2FGL J1510.9-5808cOTHER@}ø»4–W?Ëî	èz±¦@lyâ'@·€ÂhA£ø4FGL J1800.9-2407@ñ!?먿à]Ÿ¤u–OTHER@x¹'Üñf?̌èá/¡@pãÄ2ÊW¨ÁÁ4FGL J1800.9-2407gammagam?¥=B€®I4FGL J1312.6-6231c@sõY³Ð}?Ï!ٙŽÜÒ3FGL J1311.8-6230OTHER @wÞ«`ZM?Åú!íí‰OTHER@hÄû~ÿ—ÂzÆ3FGL J1311.8-6230Blazar_Candidategam|Bz??m<¼Hñ
š4FGL J1357.3-6123@skÃþ\'Ñ?ސpõ³ OTHER@pµÈV¶?ÅX;?hЌ@j*žì¿±[Âu'N4FGL J1357.3-6123gammagam?†q¬Æ`¢4FGL J1353.5-6128@sddÂø7µ?à´¬Ã˜OTHER@P	äŸH?Äz: *è@jšuÂußø4FGL J1756.6-2352@vŽ>ò"?ÝÙÓÛߺ:OTHER@=g}£Ö?Ç-0s½¯Ÿ@pÒ¤¨ÁTÊÁ¾ù>ISOGAL-P J175635.9-235215AGB*AB*|Mas|IR |*@J%_54FGL J1855.8+0150@A‰XbMÓ¿ÁvN{c"ºOTHER@/+TË?Ô¾šæü@q¿RT`ªe?ëíú4FGL J1855.8+0150gammagam?¤kiÛeìÄ4FGL J1650.9-4420c@uRz–¼?£Ú"1`ÔOTHER<@HÎÒ?ÉÅe+Qg@o—îËûµÂ1Xâ4FGL J1650.9-4420gammagam?ŽAN~é+4FGL J1742.0-3020@vf`ªdÂø¿±ƒÙÓ-©OTHER@	zèöÆi?ȟ@(Òo@@p˜"t¼jÁò¯ƒ[MML2017] 777MolCldMoC@@I'>E4FGL J1904.7+0615@DH©¼ýL¿·íêÿ'ÇÃOTHER
@	N(%ð?Æl¤êý-@qâð¸»@È7[SPK2012] MWP1G040012-001102Bubblebub@MúÐíýZ4FGL J1618.0-5119@tÄzCþ\'¿ä3™Š€!#OTHER@s^Ï?ÇýF½¿(u@nŒL˜_ÂMP—4FGL J1618.0-5119gammagam?ˆ­«ŸU›=4FGL J1620.8-4958c@tØ¿œb¡¶?k'Úæ@OTHER0@ÓŸø?Ê¿†‡ñ'@n¦Åm\ú­ÂGá-4FGL J1620.8-4958cUnknown?wFˆze4FGL J1321.1-6239@s%^~¥øM?oÒÃ(U¬OTHER@ªËèm´?ƳuRß©¨@i	,¥zxlÂz£ø4FGL J1646.5-4406@uM^³¾?éÀ̾µOTHER@Ÿbü?ƅn¤¤`@otÑ·YÂ0j4FGL J1646.5-4406gammagam?'~
ÇÚ

==> SOM_VIZIER/4FGL-DR2_prob_catalog_2classes <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  467 / width of table in bytes                        NAXIS2  =                 5788 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   56 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\4FGL-DR2_prob_catal...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'cos(GLON)'          / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Pivot_Energy)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'LP_Index'           / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'Unc_LP_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'LP_beta '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'LP_SigCurv'         / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'ln(Variability_Index)' / label for column 11                         TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR12    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'HR23    '           / label for column 13                            TFORM13 = 'D       '           / format for column 13                           TTYPE14 = 'HR34    '           / label for column 14                            TFORM14 = 'D       '           / format for column 14                           TTYPE15 = 'HR45    '           / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'HR56    '           / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'HR67    '           / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'Category_4FGL'      / label for column 18                            TFORM18 = '5A      '           / format for column 18                           TTYPE19 = 'CLASS_4FGL'         / label for column 19                            TFORM19 = '5A      '           / format for column 19                           TTYPE20 = 'ASSOC_FGL'          / label for column 20                            TFORM20 = '18A     '           / format for column 20                           TTYPE21 = 'ASSOC1  '           / label for column 21                            TFORM21 = '28A     '           / format for column 21                           TTYPE22 = 'AGN_BDT '           / label for column 22                            TFORM22 = 'D       '           / format for column 22                           TTYPE23 = 'AGN_BDT_STD'        / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'PSR_BDT '           / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_BDT_STD'        / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'AGN_NN  '           / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'AGN_NN_STD'         / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'PSR_NN  '           / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'PSR_NN_STD'         / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_RF  '           / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'AGN_RF_STD'         / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_RF  '           / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'PSR_RF_STD'         / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'AGN_LR  '           / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_LR_STD'         / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'PSR_LR  '           / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_LR_STD'         / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'AGN_BDT_O'          / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'AGN_BDT_STD_O'      / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'PSR_BDT_O'          / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'PSR_BDT_STD_O'      / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'AGN_NN_O'           / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'AGN_NN_STD_O'       / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'PSR_NN_O'           / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'PSR_NN_STD_O'       / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'AGN_RF_O'           / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'AGN_RF_STD_O'       / label for column 47                            TFORM47 = 'D       '           / format for column 47                           TTYPE48 = 'PSR_RF_O'           / label for column 48                            TFORM48 = 'D       '           / format for column 48                           TTYPE49 = 'PSR_RF_STD_O'       / label for column 49                            TFORM49 = 'D       '           / format for column 49                           TTYPE50 = 'AGN_LR_O'           / label for column 50                            TFORM50 = 'D       '           / format for column 50                           TTYPE51 = 'AGN_LR_STD_O'       / label for column 51                            TFORM51 = 'D       '           / format for column 51                           TTYPE52 = 'PSR_LR_O'           / label for column 52                            TFORM52 = 'D       '           / format for column 52                           TTYPE53 = 'PSR_LR_STD_O'       / label for column 53                            TFORM53 = 'D       '           / format for column 53                           TTYPE54 = 'Flags_4FGL'         / label for column 54                            TFORM54 = 'I       '           / format for column 54                           TTYPE55 = 'Missing_Values_Flag' / label for column 55                           TFORM55 = 'I       '           / format for column 55                           TTYPE56 = 'Category_Prob'      / label for column 56                            TFORM56 = '5A      '           / format for column 56                           DATE-HDU= '2022-01-29T22:24:27' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             4FGL J0001.2+4741?ÙùË WìÚÀ,­º<§À;J,Rƒ[À<‡éÐ2@Qì̜{K@Þ¥šXÜ:?Ë·¢C6`¿Q¬gsùï?µz'Ÿ'h3@ù-@*¡¿ë8罓ô¿?讵¬ß¿á"c+YJ¿èÙE¡Iç*¿Ú!*•»¿Þ
\¿žúAGNbcuB3 2358+474?ïÿr'§º?Q´"U
?¿˜ýèT»?Q´"U
?ïõ¯ò¡r¬?Z†e…!ß?T ÛW7ø?Z†e…!ß?ïëƒM@¿R?q66–ì e?d|²âüž&?q66–ì e?ïþXDZÞ?8ôÉ?*sƒzv?8ôÉ?ïÿ˜@ |?úéÆ>ùs?,õÓ`ÅÍ?úéÆ>ùs?ïù'ª´k?Šè–ÈR?~#6·´N1?Šè–ÈR?ïï½ñg"?j¢5‡fà6?`Br¤Ð?j¢5‡fà6?ïøag<éÚ?D÷BuH_@?Nzb\ùUv?D÷BuH_@AGN4FGL J0001.2-0747?ÞÕGqÐõÀPӅH©¼ýÀ9j8³¥´ZÀ<‡þ[@ŠÝÓÛ3î@"<½öp4?°Fc熝?¨ø\óvè?úƙ¬äÐ@ý"õ[?ïïXÌý¿á®?Ffí¿ã¤ÊOD
ò¿Úþ-b8Ú<¿èa~J2Կވ–<"AGNbll3FGL J0001.2-0748PMN J0001-0746?ïþ‡¬ Æ?!Ր$è?'…@š¤aI?!Ր$è?ïÉb#?e¨ó·â?aD\&½?e¨ó·â?ïøÈh•?Aþã)b»?OÐÞ²¸¹I?Aþã)b»?ïóà­)nc?DëÁ1îǺ?X>¥ºá©-?DëÁ1îǺ?ïý*žAґ?0bÚÞüÿ?6«ïò¨q?0bÚÞüÿ?ï°þZ{?'\ºs·ee?ƒÀyèY\F?'\ºs·ee?ïï×°Íà?jÇUÕϞÇ?`ð(‡‹·?jÇUÕϞÇ?ïäoy=6J?]ªþ0ìÝ?k†°ë¾'?]ªþ0ìÝAGN4FGL J0001.5+2113?åyèÂÍÀDužèóÀ8^Äþ¢2À;Þ¿Â"O@O
"M@bœº¶IÔ?¡î[3?ÄRÆ6ɾ@L¦CÌ«@k˛ŸXJ¿Ï® yÈ¿äeßBp<ÿ¿èÀFA,ðú¿ìoN6ĸ+¿ïÿûÎBÓ?lÏÉëN¡AGNfsrq3FGL J0001.4+2120TXS 2358+209?ï‡ÓhÈ@v?²±÷c˜8˜?Ž%ßîd?²±÷c˜8˜?ïÞçP©B?Œa3j	Î?pŒW‰Ð3?Œa3j	Î?íé%°¾¤@? ä·°IÎ?°¶ÒxÁ? ä·°IÎ?ïþ—<Èk?ÔK̹À‰?&Œ5.‹}ø?ÔK̹À‰?ï²NJ!–?""ˆ<cVf?ƒlm}8:[?""ˆ<cVf?ï¡uŠ_ƒ¸?"ºçŠØV?‡¢d¯v?"ºçŠØV?íך‹‡F?¡Ñý1'¡?±C+¥"Ï?¡Ñý1'¡?ï÷ÙµmØ?HÖóâ°)¬?PL•ÿä­?HÖóâ°)¬AGN4FGL J0001.6-4156?Ö$L^!†ÀRÓÃa@À:DOÀ1³×À<]yÞon@ —ÀÍe#?ú®oês¦Á?»xö"¼C?±ÛsÖôï?÷®·`,'@A=©-á:?í½¥|üªá¿ä«Kb©îQ¿ÑIò&ùi
¿ÑíñÀL5ä¿Ü}#Â'w¿Ïb9°ûµîAGNbcu3FGL J0002.2-41522MASS J00013275-4155252?ïÿ
ènòZ?ïÉ~9Ö?¢ò˜tŽ?ïÉ~9Ö?ïötU^Ώ?VJV¡šÃ?ST×/È?VJV¡šÃ?ïù˜E9M²?9Kiq?IžêêhQ|?9Kiq?ïü€53W_?$aMQ¢¼t?;þWN]¸½?$aMQ¢¼t?ïþ½'È4?Æþ
?$&Ô¢åz?Æþ
?ïÜíd¼?uU‡'!ª?q‰uGiå?uU‡'!ª?ïûÚ\S=?V)ä"7"¥?@—²J‡˜Ü?V)ä"7"¥?ï÷ðcÍ&[?@ãªZG-?P7Þ/~Ý?@ãªZG-AGN4FGL J0002.1-6728¿ãm5/EÀH{Râûã;À:'J7[·À<™øn;Fþ@ m#"'ÿ#?úؒ2>?Â	ˆ–.?Äõ¤îŒ@\	›Š4¢@Ï$'ҁî¿îèÌ!¬"2?Ï ¤Ð¯Z¿ÕºÀ°´¾¿ÔšÀ[¥B¿ÜÄ°ž˜Ý¿å«`"gAGNbcu3FGL J0002.0-6722SUMSS J000215-672653?ïü>^#e¥?=_êƒv-?>

ÅÙã'?=_êƒv-?ïó³¿Æ»!?X¨½éM°?X˜€Ò¾Í\?X¨½éM°?ïïC_C?R¼Úåáë?`¼íÓJôÕ?R¼Úåáë?ïõ1ÓL:?=Ÿð‰È®P?UÂ›`5?=Ÿð‰È®P?ïó®f7õî?Rjè˜üû?X£3*_´?Rjè˜üû?ïÏæ?º€?ƒž›ŸúÏô?xqŒð ßÝ?ƒž›ŸúÏô?ïÖ6ó²ä?yì@LϦ?tä†)4?yì@LϦ?ïÓéؕÐ?gzý<?vr|WÀ
?gzý<AGN4FGL J0002.3-0815?Þ:Æ$'§ÀPöK	éÎÀ;\tì;'À<¥S"'Û@ 'ev§Q=?þÚ ø2¬?Ñçq"Á?Ã7S=êœA?óM¹Nè›@ŽM¡sÙ¿ïÿú Âî'?ïþ–ÞÔ6N¿ÝüK€ª¿Úmïÿ
z<?ïú;/€÷AGNbcuWISEA J000236.06-081532.4?ïù¡@¤WZ?T™½Ø?IzýX¥…?T™½Ø?ïèé^¡?l‹^K‰?g€ÿ^?l‹^K‰?ïDŠ"0"?›"…-‡ë?—}n¬
Sy?›"…-‡ë?ïKi?Q+#¨6¥?aðG
û'>?Q+#¨6¥?ïòÕÖÇß?_éÃU«?[ÚT1t?_éÃU«?ïƒÉ•#¬ò?˜>·¼=Š.?
š·Ãu?˜>·¼=Š.?ï\:ÚW¶?¹%ûèX?"x¤±™£Q?¹%ûèX?ï•D®8j³?ƒÏÙv?Š®ÔqåS4?ƒÏÙvAGN4FGL J0002.4-5156?ìéSЮûùÀOÄþ'Q~xÀ;Á!\qÀ=dmgâg@ ÖKã*\?õ˜/6Np¦?áióïP…T?ä†Íyšö'?ÿuäô
ÿ8@/tæ±ÐG?êK7 ¦ê¿íƒgþìÛ¿èšð{þ~ ?ތ¦ æ{¿áL#ßÙ¿ïüò™åï´AGNbcuWISE J000229.20-515227.4?ïýÓÂÛ)?/wb˜Á¤p?1gð?/wb˜Á¤p?ïõíÕ'†¤?Z7ª¥&]ì?T$V¨gV?Z7ª¥&]ì?ï¾fHa?yéC?¼?€fmöê3æ?yéC?¼?ïýF؊"â?(7g÷ëF{?5É='3ÏÐ?(7g÷ëF{?ïþ˚r²z?'â$L9Õ?#FZÞ'?'â$L9Õ?ïÜzaÅíµ?t
՛NaÏ?qÂÎû\ùq?t
՛NaÏ?ïÖ¦cg¿"?Â1þÖ»]?t¬Î8âf"?Â1þÖ»]?ïù';ÁÍ?GÚ5p "?I·¸
Ü
O?GÚ5p "AGN4FGL J0003.1-5248?¾3M8±¼ÀOdüó0À:R"O…yQÀ<x|àü.º@ xŽÎ9‰d?üöYSXm?½°''¾?¬îþ%	yÑ?ó_6Ç<j?úжç2T¿éß5…
Ó¿ ©e>ž g¿áìáàZHK¿ÛY¶T»C¿ÑFÆbûLè¿äXY]ig£AGNbcu3FGL J0003.2-5246RBS 0006?ïýn}¬z?)/TáËj·?4ŒÅô+ø?)/TáËj·?ïðňñçË?a]Ýî$7?^tî7­J¹?a]Ýî$7?ïï7üä?\þÛl՛?`Èå˜À'?\þÛl՛?ïðZèGÁO?FнðCî\?_J/#†#d?FнðCî\?ïùõ¬aiÊ?BW"ȳÈ_?H)MÉà*?BW"ȳÈ_?ïÆœ©§?'¸'L0>¾?|À1Çløf?'¸'L0>¾?ïñÔìßoo?gg
op ˆ?\V&QŸA;?gg
op ˆ?ï«´ÐÆpV?w
ºúyš¬?…ËÎcêz?w
ºúyš¬AGN4FGL J0003.2+2207¿«mä›0Ù£ÀC°½ãû½{À;0')ˆ†À<w2>@­o@iBªI•?è¢Ç
,¸?árh!ýU×?ïýt³è@1¬šþ¨?úMEââ¿ä;ËB^n¿í5K Â€¿èuˆb—7?Ð;œ£º.å¿ïfKÄ#°ß¿ïþ'"oAGNbll2MASX J00032450+2204559?ï´3ßç—å?Œ%‹òëY%?'óÀŸ?Œ%‹òëY%?ï"&PªE?¥\ìûL"A?‹6kΏ'…?¥\ìûL"A?îv=é†{?–«úr¶ý?¨œ!rMK?–«úr¶ý?ï<ƒøXÒæ?‰"0hâô?˜o€ñv@?‰"0hâô?ïÃRR]E?†Ý3Í6ÿñ?~VÖÖÜà1?†Ý3Í6ÿñ?îʴ飔'?³r4|ß?£T±j9á?³r4|ß?î_Áë©?žY½}ÒÓG?ªáRi$?žY½}ÒÓG?îS-­ÿ?§_V^¨Ï9?ªÍ%1CÃ?§_V^¨Ï9AGN4FGL J0003.3-1928¿æؾ&Z¡{ÀS%.ßç[ÄÀ:‰HºƒôíÀ<w˜¢ù"¬@qŒž3‡@w°év?À½mÈ°?ϊ' U`@
D žq@œåGB	?ï¬ýw޿δ]?KDw¿â‡ôiÉÈ¿ä`‹[uN¿ë°SO2m;¿ïÿùJYQAGNbcuPKS 0000-197?ï ·Ú?©ZÕþ=¡æ?‡Ò	@©:?©ZÕþ=¡æ?ïé†TÔ~Ù?wÍ¢ÖÐx?fy«¥¯-?wÍ¢ÖÐx?ï
¿A…?'´¾-å¥é?>HöÇ!?'´¾-å¥é?ïðRxüHÄ?FÄ+åÕå?_[>h7Ð?FÄ+åÕå?ï›}}ø?ž¼,Ÿ"ù?žìII
?ž¼,Ÿ"ù?ïÞ=É Y?ŽpcP™?ˆˆpÙyå?ŽpcP™?ìŽÄ9¼u?«Ó«"<X?¿k‰Þ2T?«Ó«"<X?ïÉj'y²?lil@k?{JöU¶á?lil@kAGN4FGL J0003.3-5905?ïåòhâ+ÀL{¢£Y6À;Cü¯¨À<¼…Ñe¸Á@Ê\ñ*$@L€S?Á\¶î¿¿§~Š°¯?åýºËø<?øŸ5dæ´?ïíŠè%èMþraF¿åÉ3¿Â¿à8G¤Ú?|¿êwMt'I¿ïé\ AGNbcuPMN J0003-5905?ïñGæýR?vý1+9?]p1‡<?vý1+9?ïÕöl-z¸?ˆ:ñq¡Œ?uÉì²@;?ˆ:ñq¡Œ?(CQJ?…òŸ*ŽZ2?ˆvY¹|?…òŸ*ŽZ2?ïÔxúßüø?]RÇ/Lqd?uŠ'$0?]RÇ/Lqd?ïç¢AŸ?dýü5î=ÿ?h]¿|µš?dýü5î=ÿ?ïqü{TùÆ? |øç€ô?'Àp—•5? |øç€ô?y´ªu?‰
}¡SgÕ?‰Ö!$6Ã?‰
}¡SgÕ?î¬I(Ä"?'ªâ ®ç®?¥;nãYÚ?'ªâ ®ç®AGN4FGL J0003.9-1149¿ï,Ä­»³ÀQÄÎp:ûÀ:ՇΕú©À<¦[·¶»@³9Õs?þéÀùYó'?ÄNmRé²?Ñ[!¤?ã@
¾á77¥?÷çÔåõé?êªI¥Ò?ïЊA7õ¿Øarv?!~¿ãMDVq%Ý¿ãªèvv~â¿ïÿò"²¢AGNbll3FGL J0003.8-1151PMN J0004-1148?ï*!' &?"A/›E
?µw"¸¾‹?"A/›E
?ê?v¼0-«?Éd'£CLÂ?Ç%?IR?Éd'£CLÂ?ît½8^?œJ8)ßnÝ?¨´,|f¬'?œJ8)ßnÝ?ë¯ËÖòYh?§³©úµŸQ?Á@Ф6š`?§³©úµŸQ?¸Ú?¨K%+(dÞ?¥7¾'8'Y?¨K%+(dÞ?×/‹
, <?Òë±+(F?äh:zéïâ?Òë±+(F?ë¥68î€?¯ÒúQTi?Ák'Eþ?¯ÒúQTi?ß#¡'àø1?¿«'z\+?àn/lƒè?¿«'z\+MIXED4FGL J0004.0+0840¿ï€ž¤#ÀJ2ìž#lÀ:ߍè‹o4À<&Žà4@aÖQZæ€?ú­Yº†y+?Òè‹o4kB?Þ×e,)ª@,œü$©-@oô0¿äõj¿'{¿ë÷]>Êk?«§½ý.È¿Ùý¥ýÖ.¿í¥è\uKÜ¿ä
NÒËêOAGNbll3FGL J0004.2+0843SDSS J000359.23+084138.1?ïìéƾÑô?ceX"Þo	?c9m)5?ceX"Þo	?ïÜr…¾×?t7ÝÑ$Êä?qÆôNN *?t7ÝÑ$Êä?îñ•¨B?Žø¹G†g¾? æ¥w.›Û?Žø¹G†g¾?œ´oø?tŒ"c[?˜ÖSÝ?tŒ"c[?ïÑb"…ïª?zâïtú?wNµÌ&rÿ?zâïtú?ï_•êb‰ã?—vKuo$?"
Bºû™?—vKuo$?ì'Óü/՟?ªàŠåÒ.?»i`S?ªàŠåÒ.?î#xß©?®ã‹à?­ÈrÖÊD?®ã‹àAGN4FGL J0004.3+4614?ÆÏkì`LÀ/µ¶¡è´À:A´¶U'À<	*K-%@Hó{bKú@7<'W…ù?ÄRéF€?±:Ë^¸?ìt1ËT&É@m­3Tk<?é"€­ºc?Ò,&äñ0Ú¿æÓu}°"î¿æ6J²È¿ïÿÿ²}@¿ë
CQƜAGNfsrqMG4 J000421+4615?ïüúBŽ3?)-ðþå‹?8-ï'Ëì?)-ðþå‹?ïô¼P¹çÿ?bB#Q¾?V‡^¢-'?bB#Q¾?ïÏÊ~Ïúæ?ruIzŠ?xÀwMH?ruIzŠ?ïõ‰¢‰4û??5³â©?Tì»@©i??5³â©?ïû¹ó'o•?>C_´üÓ?A1ª)r¥?>C_´üÓ?ï̕&î+l?…+Éèv?yµl˜¸}Ê?…+Éèv?ï³Æö–l5?'Dåº:î"?ƒBaô¶?'Dåº:î"?ïމ¡N?a.¥d'ù…?p»/I!d²?a.¥d'ù…AGN4FGL J0004.4-4737¿ís?oNÀPâk΅3±À9酿ÈŒÀ<ê$Ìh@G:ï•#¾@o-d½û?´Á«†?·»Il°'@-  ôØ@½Î°|µ¿Öš¢bë݉¿äà}ƒ¹^¿æwž™¿ã%ªê#õ©¿éˆÒ!Š_¿ïÿàU?ÍuAGNfsrq3FGL J0004.7-4740PKS 0002-478?ïþ><ü‹?$¯»Î@0?/|g1
?$¯»Î@0?ïöòäþ5¿?U'^2Ä?R5Ýá¯?U'^2Ä?ïêJ\Ö«Ú?eŽu
÷?eµ¢òZfX?eŽu
÷?ïÿô6>ùiIœæ9Ÿ?'ô>tb>ùiIœæ9Ÿ?ïý¯ßí?);àAZ­?2•½?);àAZ­?ïÛñÚ?uj}b±o?r7ŠãN?uj}b±o?ïÛ&×°*«?v~àϛ۪?rl"Ì?v~àϛ۪?ïÿ«Žø?F‹2€€?ª"Ȳ¡¢?F‹2€€AGN4FGL J0005.9+3824?﵆`ƃ À7¸dàÀ9œSÆP±ÉÀ<"Çȁ@p!G£X@j˜û(¸?¶Ã0òZ¦?ÈNÇ"é¹í@ô±î$5i@
LPóãg¿Ë&'¢È¿ânyZ^ñ'¿ê
ªB^Ia¿ëD§>ȽŸ¿êg <¶j¿ïÿüÉï£AGNfsrq3FGL J0006.4+3825S4 0003+38?ïÂÛõ@Å?¦É®ª‡?~'u|p¡M?¦É®ª‡?ï獹¢´²?hßú+ær?hrFŒþ6?hßú+ær?ï5ÔgÇ?ƒ2´äGð‰?‹òŠß]]?ƒ2´äGð‰?ïÅ\±do?cDxÅ?}Q§lÚ?cDxÅ?ïÅãI;h?zL.S
çÊ?}[Oîh?zL.S
çÊ?ïŽm+c?•qdÀ/?Œxû($ÃK?•qdÀ/?î3Ø̬¸Ó?Ÿ$iÞ³-?¬Âs54r×?Ÿ$iÞ³-?î)ùPìà?–x·n89O?­`jóųI?–x·n89OAGN4FGL J0006.3-0620?êe¢@ÝîÀP¨òù‡@À;/#Dže/À<­\Ï
ï­@·-¶œ‰¹@ØTÛ#§¥?Í"ÆÔeH?ųNáåbÆ?õOl@!ð!慿ç0Ýî]@M¿·?ï.K—Ù¿ä'§
öbȿݶßz¤`ó¿è:Ë­èÛ÷¿É~-W|AGNbllPKS 0003-066?ïþœzõi¤?Æköÿim?&8NêþèJ?Æköÿim?ïïÅßȨ?d	%†_õ›?`ë9ýÛ@6?d	%†_õ›?ïé¬Êv–?htNW4©?fS5ŒGÚ1?htNW4©?ïû͝FI?&íçá\­?@Ɋ÷#€±?&íçá\­?ïýP'1?8PÄpEëŠ?5¹â¤üT?8PÄpEëŠ?ï¡™Õ?õÉXn?‡º™»Ê¾L?õÉXn?ïÇGš"Œ?'¨v¼­?|qÜ4'Õ?'¨v¼­?ïëAªDa¯?VÏo¯ßWô?d¾U°Ÿ'I?VÏo¯ßWôAGN4FGL J0006.4+0135?ïôEÁ͌³ÀM¦&þq‹À;'Æf>À<¨Ð©*0@t×#x€?ûÚЛŽf`?ÕaÂÍÅp?ԍŸ½~ü?ü
9‰Ž‰›?ý[ÛU{²~?é&>ÚH¶?Ž"Ñ,û-*¿Õ¹¼å#/Û¿ÝOõ`¿³_¿å¶³ «Ü'¿ïëñUBQ´AGNbll3FGL J0006.2+0135NVSS J000626+013611?ïøVM?B‰=ˆ2ºá?N¦Ì¼+ç>?B‰=ˆ2ºá?ïÅ&Bèe?ˆ)Eºº?}lÞ¬Éy=?ˆ)Eºº?ïµÔ?æS?xò×í¢
f?'¹ÊþÑI?xò×í¢
f?ïq'ÍØÄ?q{ÕŒð,?'Þo¤'?q{ÕŒð,?ïôHŸ+(ù?RìÂVîK'?WnÁÅ*î ?RìÂVîK'?ï³®åþn?¢²þß%?ž)Š+×8$?¢²þß%?ï†úY@'?ˆÐðo™Ý?ŽAi³¡"g?ˆÐðo™Ý?¹qs?"ÐJµÏ½ê?®gvfüÒ?"ÐJµÏ½êAGN4FGL J0007.7+4008?å]×Hs-ÁÀ5ùÙUmÀ:Ë
Tí˜À<fߥ¥@"Dˆ›¡?ÿ¿Å}M3?Ãß4®]uý?ÆøĤ•@á*¢jùs@	ýÛV}e1?ï6è)I¥e¿Ý'‡"-D¿ãœzõi¤	¿ØëÚcä+
¿êWAï8²¿æÞ+	Ë[AGNbcu3FGL J0007.9+4006NVSS J000741+400830?ïú*Èx'?Ca«á'0?GTÞÕM·n?Ca«á'0?ïît>6_?g¶`S™±?a‹ÁåÌ Í?g¶`S™±?ïØéêP&š?uºÞÇÐÖs?s‹
Á?G?uºÞÇÐÖs?ïÚfét?Už«Ijè6?rýLrz•û?Už«Ijè6?ïé¯ÙÌåv?g›,ð½µ?fP&B8ф?g›,ð½µ?ïȖ¿"N?oöæÜW?{´ y¾M$?oöæÜW?î¤ÆM€‰?Ÿç$Šû{t?¥³ž\Þr?Ÿç$Šû{t?ï}nô2?sY—±]>?Œ ¤Bóx;?sY—±]>AGN4FGL J0008.0+4711¿ãQgÜ]8•À..¥.ùÀ8¹¢‰à¿À;§=áâއ@ÞTû½?þÛ«©gm?¦%"¤DÃS?´A﹋Ò\@®jv–_R?ýÉ
mAL¿ßÚ£}ɿך/ ~û‰¿àŒ
ÑyÛ¿ÛsËßgD¿ãéoÐrs»¿æ3R3ÐèAGNbll3FGL J0008.0+4713MG4 J000800+4712?ïÝIÃÝ(Ô?gù±'òÙ?q[
}Ë?gù±'òÙ?í…"¨=÷?¹®º_"Ae?·ëÓduÞD?¹®º_"Ae?î´é3éD? ßZò?¯Ä±oU ¹? ßZò?ìƒVà?	?™"fW.t?»åKþ¶?™"fW.t?ïRH¤ßrí?'¢×<?•¶ë`¢o?'¢×<?ÚÂÀ¤ ]Ù?Ð⫀÷·1?➟­¯Ñ?Ð⫀÷·1?íºtâ?£_ÆþÔ?²,_y%n?£_ÆþÔ?ÞÖ+¼'ö?·õ#*—ý9?à"ê!¾¹?·õ#*—ý9MIXED4FGL J0008.0-3937¿ïžÈ6SèÏÀR¥UGZ1¥À:½ÆßîÀ<xLuúX @Ñ"³U@+ã	O4?ͺš›!Y?Ú
‹t<è¿@»íx:¤@7Š:?îãË\4¿á롃rç¿éï¦`ÒRÉ¿ë:Ÿc2)¿î_ÌqæÍ¿ïý
':"AGNbcuPMN J0008-3945?ïäõ˜Ñ{;?ƒzk	?k
gižÇ?ƒzk	?ïÅ4A}V?ŒB{?}eòúH ?ŒB{?ï*Ÿ‰Œu?‹xÚq?š®†?]?‹xÚq?¿'8?pZdˆìQe?‹|ÝÙáõ?pZdˆìQe?ïµKOÎc??'ɉ"j6?'­,Ø_?'ɉ"j6?ï=kî&‡?£(Y5\uz?˜R'?/?£(Y5\uz?íi£)n?¢E''f½?´·ç%x?¢E''f½?ìPğñfN?¥Ýõ¹ð-?½yÛt͐?¥Ýõ¹ð-AGN4FGL J0008.4-2339?ïÿÿàSÀSì6ŸÏ=ÀÀ:Èeü´%À<{¼Ñ­^@!"þäÌó¹?õ•ôäC?Ñm>Fâ"?ÑͅC÷%¼@xCx%@påÆBð¿ïîÎô©‹?ïùÑb]Ã*¿ÆJ>¨nڿǯ³ ÿ)¿¢/¿œsÏ¿éÍáõ¨äAGNbll3FGL J0008.6-2340RBS 0016?ïûcDŒ»©?;J‡:ÈG'?Brí]w¤>?;J‡:ÈG'?ïèäw…¿ê?lM–NŸ?gˆ=Æõö?lM–NŸ?ïÅ©d_G†?z,1=8~?}+MêyE
?z,1=8~?ïöMs©?CÅ3!túã?Sñd—"^ß?CÅ3!túã?ïõŒ‡Ö?TêÿávÐà?Tç×_åÓ5?TêÿávÐà?ïBŠ5šä?›"¶­3{ï?¯]dÚ×?›"¶­3{ï?@ô£?†ë[zœu¹?‡Pﱩ/å?†ë[zœu¹?ïà¬<«ÏI?g¡'5Ê?oSÃ5ô'‹?g¡'5ÊAGN4FGL J0008.4+1455?ã¤Rò/ ÄÀGVžšÀ:J‹¤äPwÀ<fjbti^@¡Úõr?ÿÈ+}\L?ÃÖÅIُ?Ä|í'hr°@_&¼,k™@Ðÿ¿EÑ?ïñÁä;~[?ÀV5VNb¿ÛAÅݚOw¿àðž'ú¿ât"Ì¿ïÿÿ)@k*AGNbcu3FGL J0008.3+1456NVSS J000825+145635?ïôÜ-gí$?O]ç¿¿ô?VG¥	ªÕ?O]ç¿¿ô?ïÇÅ(5¿?ˆ¾Ÿ"õ—T?|lˆg?ˆ¾Ÿ"õ—T?ïÒ4ê‡6¯?sK'olM?v劣§xv?sK'olM?ïE°bLÀ?w°Ô&½îà?—Ió±@"ê?w°Ô&½îà?ïÃÍ×0©?sVOŠ%?~pwŠó³?sVOŠ%?îÿfà'À?¬-ýeÝ.¹? 	žA!?¬-ýeÝ.¹?ïVáÛZb?ÏÀÍ.)?•,CÁ%Ê?ÏÀÍ.)?í!81IÏ?œ›³µÝ–?¶ö>u±‡ø?œ›³µÝ–AGN4FGL J0009.1+0628¿æ+xïÞÀKo$cŒ—SÀ9ö™"º]À<HßݵR@(É°7À·@*¢jùs?¶½'é("3?§_¾EdR?ñÇ=áâއ@Œ@ž'?鸞—@¿ÌGNž·Ì¿ãéˆà
ò1¿ß@?
Vñ¿á¨–¾•¿ßç¢ünÐîAGNbll3FGL J0009.1+0630TXS 0006+061?ïýC	Ñ ?%[…£QŠà?7mç_]Ì?%[…£QŠà?ïîO˼£×?bч,ë­?a°4~up?bч,ë­?ïôBDbI?`³	b'?W{ÿnü]A?`³	b'?ïè·=æ·Ò?OIš\pñë?gHÁù«ÆL?OIš\pñë?ïúÑfdŽ?9Æ(i
ß3?Gø¹È¦q?9Æ(i
ß3?ï¨)¾Ñs?Ès}ÒÉ?…úõššwD?Ès}ÒÉ?ïìãA¬Á?sÈ,)(Ã?c¾¯Ú?sÈ,)(Ã?﷈9lT´?l3Oî–ÕQ?'ñ¦ú–ç?l3Oî–ÕQAGN4FGL J0009.3+5030¿ïÊMùTŒ—À'›oâæê…À8mKrÅzÀ;•L''Ù@»-݈ܳ?þ\Ü_? Ï¯Ù¡ò?¯ãçñkg­@§óþiýË@˜p=Ö?µ,ü€kö¿Ý€Á›ì/>¿ày`^dL¿Üdµ÷ž1¯¿ãL
Ìsá¿á¡ê€¼ÓÛAGNbll3FGL J0009.3+5030NVSS J000922+503028?ïýÓ\€Uó?*7Ÿ†?1eFµ×?*7Ÿ†?ïî;Š£?jKw'ë¶?aáñôäƒ?jKw'ë¶?ïãíèÑ:E?tyw§Œºy?lv?tyw§Œºy?ïû!ˆÞ,é?-ä¡N±0?Cy܃ÿï©?-ä¡N±0?ïþM³g  ?#Ê+WËÔÝ?+$Éè&÷´?#Ê+WËÔÝ?ï«q̇=Þ?"¹r¡	ó?…#Œëîø‡?"¹r¡	ó?ïïú+?r˜½ÐW?`ë< Ý
>?r˜½ÐW?ïô›¨'…Ô?FR…Ÿ¼š?VÈ®mØo?FR…Ÿ¼šAGN4FGL J0009.7-3217?é3ë¿×ÀSå¶ÃvöÀ;
Ë
Tí˜À<ÄFdh_e@I%Â1hX@¸¸]©ÿB?NjÑÅZÄ?Àq<XJï½?÷­_™Ã‹@л¸¨Rš¿ì)ˆ$&Oö?ïþ"4­†¶¿Þ5»8OÒ¦¿ç0ý~E€=¿Ùm"Ãqx¿ïÿ÷Âé±AGNrdg3FGL J0009.6-3211IC 1531?ïý_½»óó??–—û^?5"ÓIz??–—û^?ïÖA"AD?…iyã"/??tß5èÊI?…iyã"/??ï†h‡Ü`q?‹¡κÞo?ŽeÞxG·?‹¡κÞo?ïõœQ?Aî-Pô?UâƖ¢MX?Aî-Pô?ïñD©zã?hGu­‹$?]wÚ÷AÉY?hGu­‹$?ï>Nžc?£J·%{µ?˜6,0jÕ?£J·%{µ?ïHãâE¸z?'ÁØÁ¼g>?–ヺ¸ŒÊ?'ÁØÁ¼g>?ïÑXä%b?l–œÀ?wpӟ[?l–œÀAGN4FGL J0009.8-4317?ßà‡ÉQ\ÀQñíåKIÀ:Ì{¥'Ì À<¿¹!]¹@¤ð'õJ@_¨†œg?¿ŠŠ2‰~?–ÃEÜÐrk?Ù|xl·c@¡d½Cî?ïý7˜ól¿ãGêüó¿àeê«%)¿ãŒÿÂÃ^¿ÊËîÖaöë¿ïünEWøåAGNbllSUMSS J000949-431654?ïþ?tÓ?÷t<Ú?&,	!׋+?÷t<Ú?ïöT&0?UTán†:?SW´m¦˜?UTán†:?ïðt†²¾?aÐùHÖ"?_ògÀsm?aÐùHÖ"?ïÿëG¿»?	Aë£÷1O?¢˜†©ñ–?	Aë£÷1O?ïýà˜±'4?/L¶®±mM?0û:>§•/?/L¶®±mM?ïÜYA娑?t'fYHÄ1?qÓ_:;'?t'fYHÄ1?ïñ¦flØ?f³ÕVŸy!?]Ö³%gà½?f³ÕVŸy!?ïý­½Æ}?):zR"¾?4'g_wl?):zR"¾AGN4FGL J0009.8+1340?â쀈óÑkÀGüU\Rç.À;W
F9 5À<Ÿ"Ì'úò@5 t-Þ?ÿ1-=¾§?ÝI–a€Îr?Ìô@ÚÖ?ñDœ¸2@ý³Š²K?ïâu@ýA¿ë¢&Á	õø¿â¦2ƒ
¿×Ï`ۍ
¿æÊf¿ïþ^	 '²AGNbcuRX J0009.9+1341?ïù¬ŠÉï?Aæ—yyÕ?IMÖé!·™?Aæ—yyÕ?ïìXß%{?g†€ÙÍoï?cp§AÖIJ?g†€ÙÍoï?ïÝt2_M?h·À4†Äÿ?qEæÝýÉ/?h·À4†Äÿ?ïí^>ñú¦?F24¸ò
?b¡Á!C)Ê?F24¸ò
?ïúo?h?C‡ "Jll?FCÒrãIw?C‡ "Jll?ï·¸<Jï?WY€idÐ?'ðù=ø@?WY€idÐ?ïÅ
¯E?€¯2˜8²'?}wú¬fÍU?€¯2˜8²'?ï±TiõÎ4?r<¦œ/ú°?ƒªå'Z¦æ?r<¦œ/ú°AGN4FGL J0010.6+2043¿îæQ¶´ÀDk&¿‡jÀ:àÛŽ,~À<W÷7Ú@ïùR¼»]@þÜ~ñw§?Ê9R‡w'?µ|Û·Ì5?éðüVþ—@
ZɈ'?ïÌöˆ‡ù^¿à‰Éb4'¥¿æ8a¦
Ec¿äyïøK¿ïý÷è‰ø?ïå Jù"–AGNfsrqTXS 0007+205?ïþ èéõ
?'̂?"9?-ñqFKÊÞ?'̂?"9?ïòìÐÃ?Yf¢íœxa?Z'ÈDGš®?Yf¢íœxa?ïÜt59¦H?p´§¼Bù?qÅå|™ø?p´§¼Bù?ïüQÉ<?% ÐMFIå?<y-¦X?% ÐMFIå?ïÿm'¦?žÉ]ê¨?òVd´·7?žÉ]ê¨?ïÇØے§&?'¶ûßqۉ?|'.m]?'¶ûßqۉ?ïá'ï'âê?{Qÿ†ÚŽ?nmǞõ¯?{Qÿ†ÚŽ?ïñËÚ^…Ç?MØpËÔï¶?\hK‡¬ ÷?MØpËÔï¶AGN4FGL J0010.6-3025¿åba'àÀTÞ?»×²À:-úNwÀ<‹3b-Â@g@õ¼@$
COàé?·Œ~Óð'Š?»)Üâ‹S@R'IðäÚ@Éh>WÔ?é¡ªñA¿âLý|íç¿å9ΛÙæ¿ë÷…¿â¨°"rпïÿ÷fÔJpAGNfsrqPKS 0008-307?ïþŒéO¡?%ýו€j×?'?Õ¤ñW²?%ýו€j×?ïëÁþxҋ?nôȵU'Ë?d>P3µi?nôȵU'Ë?ïסˆEÅ?z7"ž"€?t/|X	é"?z7"ž"€?ïþÃÀð±À?gùÊ\C?#Ãò&Ž?gùÊ\C?ïþª=9>?"¶œ!°?%_è
±4Ï?"¶œ!°?¸Ls\?"Bí3¡L~?Œ^'óÂ`á?"Bí3¡L~?ïÁ|¹ÚÆ?'yºaÖUØ?Aö"DhÙ?'yºaÖUØ?ïü´ì†P'?0)z{d¸¹?:Xšºš´æ?0)z{d¸¹AGN4FGL J0010.8-2154¿ê'ß9РÀSÙ¡ß¹8›À;3ö Û­:À<»:{&@jˆûf¾%@nLa…V?ÃÍzFÃý¿«H^éop?æGߒ¢."@ž¥]òú^?ï߂ˬç¿Þšù*3°¿æý¾Ý ¿äƒž?ò¿à¥R©®e¿ãûxFbºàAGNbcuPKS 0008-222?ïýÉ]<Ø4?&®'‰pK?1µŸ?&®'‰pK?ïì¹K]?hêœïw
:?cF´ÕÂ7E?hêœïw
:?ïï¨\È?`ò
|k›?`WÿcT‰?`ò
|k›?ïûí´ÁW?(M=Ìç°?@K `xK<?(M=Ìç°?ïûzëê°t?A;R3üù:?BQÐf"?A;R3üù:?雷MµÚ1?Ž18=Ppð?†¬×Ð?Ž18=Ppð?ïܑ¼^J?vàµê:?q·!èþž»?vàµê:?ïè)ßnÝP?[ü´Ϫ?gÖ e'°t?[ü´ϪAGN4FGL J0011.4-4110¿äDٍÇË©ÀRn!ÄuæÀ;D°P$ÜÀ<³@ý R@v^í T^@(z§f?ÐѦü-¸u?ÄCcW`€?ðö›r¸?ù©«?^dº?ç"0ý
'¿ç§0@9«ó¿éPÁ^.´s¿ä¾cþW3n¿ïý
ýn«.?äógkI$AGNbcuPMN J0011-4105?ïõ•ó".B?P2ïŒÿžO?TÔ¹fëÖ?P2ïŒÿžO?ïÏ¿4Öò?'g/´Ú…?x e¯Àû?'g/´Ú…?ï›À>/KÙ?|?šu½Át?‰ðwœ¥°?|?šu½Át?ïç±ó‹0(?TŠ@sp
?hN›KwÜ?TŠ@sp
?ïíô4'¿?f5¯1ÙÞX?bäš]á ?f5¯1ÙÞX?ï+è(råÑ?®W"G'i?š'úïëwí?®W"G'i?îúÐ.ñ?"4ι˜ñ? ^ÞFl¬ï?"4ι˜ñ?îӐÝC¤?•¬^ìj9?¢Îæðs÷È?•¬^ìj9AGN4FGL J0011.4+0057¿Ó?d©ÀN&¾œˆacÀ9ô–Å©ÂÝÀ<N­\Äüõ@L€oüè@IHÜä.?»ÞÿÝp^?¨:g³?êþ;¹ÿk@ö5¦Õí¿Ýù¥ÞÍ«¿å溌¤¿¿å×w¶á¿Û(RšǦ¿ëøV¿ïÿójÆGxAGNfsrq2FGL J0011.3+0054RX J0011.5+0058?ïý!k"6?*ªwÌjÞ?6ô¦jÕÌ?*ªwÌjÞ?ïñ‹1R?bx•¢p9?]âêZÑ+²?bx•¢p9?ïá1eәp?séYñ$˜?nΚ¨ k?séYñ$˜?ïþô,À°è?ø¤W¿ÚÎ? ½6èkÎ?ø¤W¿ÚÎ?ïüڟ?73µ[²??§×ü©ÿÛ?73µ[²?ï¾Ëƒy-?†Œ"¨ÞÀq?€M?hÀœ´?†Œ"¨ÞÀq?ïåný—M˜?v–ß™oàˆ?j'y0ˆS?v–ß™oàˆ?ïýÜÊ5ï?&˹¯þ¸L?1›@ ñ?&˹¯þ¸LAGN4FGL J0011.8-3142¿ê¶—;ùÞÜÀTõƒ¥À;N²™DàÀ<ÓNáåbÆ@ 9ûIaó»?þ²ÜæöC¿?Ì]TS:?±]íÆídÈ?å>lý"O°@…'¤Ø'?Ú%â]ã°¿ëÚúWI'ñ¿â€
¡©2"¿ÔÞ¤»Œ¿Úyb&ñ†¿âd?Ÿþ¶AGNbcuSUMSS J001141-314220?ïÿG֌G?ì›Ýs;??Ô|?ì›Ýs;?ï尗s4ç?yB¬´¾¸?jOh¨ï?yB¬´¾¸?ïÍaL—«?€±îðm?yO|ÏeV½?€±îðm?ïþ²šhîÎ?ær€€3{?$Ö\`ñ@?ær€€3{?ïÿtrÿ¸?d÷µeP9?q§nXðJ?d÷µeP9?ïvùtܲ?™ä#­8šÂ?' Ñ_BUœ?™ä#­8šÂ?ïÐá9@h{?'$óüÙT?wcrY¦r?'$óüÙT?ïü5Ɣ2?3gTeØŸ?>QÉnûÀp?3gTeØŸAGN4FGL J0012.0+7043?V+ìÔ@ 9(| À:Q/|À;Á2š†ÿc@
žÇ2@=v?ø="?¾Ñ8Ñ¦Ñ?Š›ÓRt¾?Ïý"ÀÁќ@tâÕø›?ï^0§g¸¿ç
µÂÅ¿ç
ˆ~¿¿ä'1}Ñg¿áEÅÜïüÆ$<kAGNbcu3FGL J0012.4+7040TXS 0008+704?ïü¥M_|?.IƖ._T?:Ô¡{²Ã?.IƖ._T?ïò´i?]ÛÊ`÷¿§?[õŠ4¾ý?]ÛÊ`÷¿§?ïïk5‹°«?T§Zé+?`"ʤiÜ\?T§Zé+?ïñôà£T•?AS~4×_?\>=¤ç†?AS~4×_?ïôD|J˜?R{'á&
?Wõw6%Ž?R{'á&
?ï|̞œ?'0Ÿ¸ #?ˆ ÌÎ+Dó?'0Ÿ¸ #?ïÎP"õ6?v¸"|å?x×½˜Èß?v¸"|å?ïÀØHµå?i\Þþ®«?"ÛúE5©?i\Þþ®«AGN4FGL J0013.1-3955?éf–õÀR»ê šª;À:¼b~À<vA
çI@½PdÇTé?þ¯¼†-¬?¸|)ò?½€{:ˆçñ@æ"FsØ@øv3xR¿îÄ"YFB?ÜR–»B᧿ཨ6ëN˜¿ßɯvz° ¿Ü¢‰'JG¢¿ïáGãÄ`AGNbll3FGL J0013.2-3954PKS 0010-401?ïýŒHUâ¾?*».½·ô?3½¼ªšÅ?*».½·ô?ïð üö?aכt†B?_¿Ó§Hå?aכt†B?ïãsðñ!ô?rø]~ö''?lŒð¡{Û?rø]~ö''?ïïWAï9?GCãeÄR?`¨ÿÜMW$?GCãeÄR?ïøl?e½ì?F¦S@|/á?NO´YW×?F¦S@|/á?ïÅL÷ï)2?…4t"iå*?}Y"%ø
á?…4t"iå*?奈ÚC'â?Š¤†°Ô`Ï?†ÜÉyn‹?Š¤†°Ô`Ï?ï­j|¶)?u[¿
[?"¥`æäiæ?u[¿
[AGN4FGL J0013.4+0950?妈vËR=ÀIóƒ@'À‡À:þ¨ø².À<Y·ø)qé@ (ÇÉ@ёW«¹?ÂGÞ;	@q¿±6"K~®‡?ççÛFSË@¼ë-`
'¿æt~7¸~¿éGúÀ{ٿ♅CÛ!¿Õ!â"o¿å®‹cuñ¿È2G%˜âAGNbcu1RXS J001328.4+094942?ïþY56©Æ?ý§±ˆß¸?*l°,"­c?ý§±ˆß¸?ïîWÀ¯¼?e6m¾+Õ?a¨ì{Éd
?e6m¾+Õ?ï÷®a@¦}?`	ÿ;>¯e?P£=y3¥Ð?`	ÿ;>¯e?ïüP¬|›?'=È{B
M?=zž(þJ
?'=È{B
M?ïüóԁ)¿?1iI›<?8aZ1²Xû?1iI›<?ïÁ?qý@?ƒò/¢M?~`%U4E?ƒò/¢M?ï÷ª•"%?i$ÅlfFº?PªÕ
óËØ?i$ÅlfFº?ïãn²:O\?a¢àae\?l'M–õô
?a¢àae\AGN4FGL J0013.6+4051¿áËsEòÓrÀ5svæj±À;ªáÀyØÀ<ž&~ïÊ@â¦J,@ÓjZç­#?Àz•ÈSÁ¿ª4
x¹z5?êE&z¾@@Û+'9֐¿ê ÛýÂ8¿Ð_f,"ÃI¿å¯wè]L¿âF(mÝS-¿ëyð¼–ä?ßú1Ÿ_VRAGNagn4C +40.01?ïüáx'?4¾ÖŸö^M??ô{8¡Œ?4¾ÖŸö^M?ïóöÀÍK^?YùÞ:Î×?X~"#ó®?YùÞ:Î×?ï¿H-øí?€(<zPÉ\?€-ô¯'ÈÑ?€(<zPÉ\?ïø|(¤—?5j¥t§Ò?N`h¯­C?5j¥t§Ò?ïð,X"«Ñ?\GIvÒô?_§O‹í­B?\GIvÒô?ïÈÞ6	Yù?ºÝO;¨~?{äÝÆ_l?ºÝO;¨~?ﵫêÃDŽ?†'|_d#?'•U•`â?†'|_d#?ïÇø¯©¦W?oRuì‰â?|¨6ۀd?oRuì‰âAGN4FGL J0013.6-0424?䝠ËxJ%ÀPcgM3HÀ:îÍ´SYCÀ<9òYNP@gzÃ?°D@Zþ¾·`T?Ԉx47¿±ÆÆ£gùŽ?ì´Ê(,o@r! 
Ò¿ì?"ÿ%åm¿ãm•ßû¨­¿êÑà2_¿ÛÄBÚÆ	º¿Ù›pß;9g¿ïÿÿÊPËAGNfsrqPKS 0011-046?ïü!Üý$6?I °¢K?>ñQޞS?I °¢K?ïìV\zv¶?i1kAp?c©£ˆ	å?i1kAp?ï肈0½?gµ/+G?g}w©t¢þ?gµ/+G?ïüÏ.¯s~?%Œ;´Å'ê?9†ˆ¯ÿ·t?%Œ;´Å'ê?ïñ]3sA?]ú"ÿƒ²Â?]E™H°,â?]ú"ÿƒ²Â?ï¨t$-öw?ŒôŒW²[—?…âöê3ŽC?ŒôŒW²[—?ïÔ¦ˆÈï{?|B¾ñãÍ?u¬»š(jl?|B¾ñãÍ?ïàzƧ2?cþ'•ŒûA?o…9þ8©?cþ'•ŒûAAGN4FGL J0013.9-1854?æ
ê‡PtjÀS…âlvKÀ:m» ÒÞ_À<…©²'b@K¶¤l[?ÿH‹¤äPw?¾`»ô?£Yÿ$ãº?æQSåZbL?÷¦è\JX¿¿êÝ´±M†¿Ã ÝE?û¿Ýc-˜pû¿ÝdŸý5ö1¿á—¬ÂkJ¿ÜFàd.RÏAGNbll3FGL J0013.9-1853RBS 0030?ïû$º…³š?AÙáþ­
h?Cm3i()?AÙáþ­
h?ïÞiLŸÀÐ?{^Ý©'É?pËY§àˆ?{^Ý©'É?ïß?PLôz?r•2r<4C?p`W¾âó?r•2r<4C?ï×&ܧz?]¢1 s ?tl'®R¶?]¢1 s ?ïóeŸ¹e´?TëE_ði?Y4À»ïG]?TëE_ði?ï~S"-¢X?•:ˆ"_º?5¡*ìð?•:ˆ"_º?ïȈ:}Þ?'DñÞ?{»¸
dæ?'DñÞ?ïDä`}?†+'"'¼?—c5¨?†+'"'¼AGN4FGL J0014.1+1910¿ãÙØ<ÜCÀEiÕ^kÆ"À:¤z
ˆ?À<ƒ€!ùO@ Y:ƒßs@<t$•?ÈùùUÁÓu?ÉD‹ÑYú@—Oµò–@
{I.óŸ¿Í-÷I£4¿ÜÔì@…4¿ãŒ'Á)i¿âñ¡§Úû¿íÇçÀn¹¿ïøðiŠAGNbll2FGL J0013.8+1907MG3 J001356+1910?ï˜WlI!?´¤‹@3£{?‰ê8h]SÇ?´¤‹@3£{?ïñÎå^q®?`Äøèò?\b5Ç
£]?`Äøèò?ïc$ϺŠL?`µOí#?"›fRn?`µOí#?ï÷_»…j?6´vý}è»?Q@‰cê«È?6´vý}è»?ïñå:®?W£¡ˆë?\5™R©?W£¡ˆë?ïǏ÷'?ƒºœoÌŒ?|8p€…F?ƒºœoÌŒ?ï
âPíƒQ?– ˜=-p?žCµÝ(+ò?– ˜=-p?ïáÝJsk³?[§wOîn?n"µk˜
­?[§wOînAGN4FGL J0014.1-5022¿ï¡rDQNãÀPlwÄ\»ÃÀ:"TýˆV{À<»à'ó@ŠÏ«úDT?ÿ{7(‹9…?Á
!«¡"?¡7öx±?àj|«LI…?ç¸øaœæ?ï(þûž¿éˆ—~6fÄ¿Ù#Ìhù¿¿áÝßÊÖS¿àg"Ý—ö+¿àp¯*$–¸AGNbll3FGL J0014.0-5025RBS 0032?ïúN±z7?A»¼¢ó"H?FÅ:¬‹?A»¼¢ó"H?ïÄi(¸…î?Œ¬AÂ5?}ËkÁù˜à?Œ¬AÂ5?ïÖ	 ×jN?}Þö>Äå?tû/´—,?}Þö>Äå?ï*²U?vËßIª'?ŒµS'Š¾?vËßIª'?ïð
°÷Èé?cÝ盧1?_êže¤~3?cÝ盧1?ï¾Rû>i?­Ù¿>7ÖØ?ž(5 ˜2ß?­Ù¿>7ÖØ?ïכ{'=™?}ªæ"ï•?t2BS~ے?}ªæ"ï•?í·ª>‹»? $
]9?²B®­©? $
]9AGN4FGL J0014.2+0854?æ1'³ÆbóÀJm²•éâÀ:ÆL²`9üÀ<$ü.º'¯@p.#(ùô@á~4¹E?ÄBáÑ윿¢ÀÛkT?Û¬ƒå@ýTƒ™¿ï9¡v\Ô?ïùƒyœ¤¿åñ™ O–@¿ã.IW¿ïÿùŸé"Ú?ïÿ·ÀÌ
ŠAGNbllMS 0011.7+0837?ïñƒÍÏ?[=YŠr?\ùÙòcƒ?[=YŠr?ïé_ÚÜ"?rÑEÎZ‡[?f $úÀë?rÑEÎZ‡[?ïF.Æo™?mL¦Ð""?—:')uÖW?mL¦Ð""?ïòî艀?H@>ȤÐ?Z"/a5ß¿?H@>ȤÐ?ï¦Þ87²?Š¥Ÿ<åœ?†}g£?o?Š¥Ÿ<åœ?ï‰ÚVD§œ?˜ki@ǁ›?‰jkf|ø?˜ki@ǁ›?î÷|.,kÌ?"uì@Y? ˆ=9C:?"uì@Y?ï~éF¢s)?†ŽÁdU?"×&Š0Û?†ŽÁdUAGN4FGL J0014.3-0500?àµRnÀP‹¬GG"À9þ!e«U"À;ó×Ûô‡ý@ÜÀ? ©Ù@Öæþ¸?¾á@øÔ2?¢hEÿ/Ý?äÓìŸ@ÀëNB-L?ë'm{-È¿ÚíÎm¿è¬l°{¿Ü;ŽK‡½Ï¿åÆ û;¿ðAGNbcu3FGL J0014.3-0455GALEXASC J001420.46-045929.1?ïýpÓªü?&³§ýmîz?4yg/x?&³§ýmîz?ïîˆS¡Þ?d'ÕÎ\Ә?aw¬}*±Ý?d'ÕÎ\Ә?ïí"ë…?e)4ŠSß?blè"ËR?e)4ŠSß?ïö2,ÿÏ?:×B6JÂ?S›âsB:?:×B6JÂ?ïûjöݱ:?;a
T÷?BT#µ"'–?;a
T÷?ﮝ"ÐÜý?èïk}êv?"XšÔ·¼Â?èïk}êv?ïÖ獘Y~?zwô—ÓÆ?tŒ9M@]
?zwô—ÓÆ?ïÛ©=ÈÚÇ?`O%E¡'A?r+`ú–\—?`O%E¡'AAGN4FGL J0014.7+5801?ÐÃrc¯ZÀþ¡]³9À:ŒäxºüÁÀ<Uò#žjº@"R·Áø³[?øÙ<|ˆÛ?Åå¥vF®:?Ɖ·ú,×O@A&PÍ@‰¡a¿ïá@Âgîý?ïê'ñ¶'!¿Ó~°_-âç?­Ì8þ#[û¿ÔÜX[
葿ߥ83M4AGNbll3FGL J0014.7+58021RXS J001442.2+580201?ïý!ÍÉæ­?/ˆ'Ÿg©Ü?6ñ'mèHq?/ˆ'Ÿg©Ü?ïéœÆl,ñ?qX²
:s?fc9Æ­Fr?qX²
:s?ïðLdQµ?Jԗ?€µ?_g8XÕn?Jԗ?€µ?ïéÅhKæ*?P¦°^O<8?f:—Ó¶=ò?P¦°^O<8?ïøNšº"s?Gæþ9{³r?Nŕp…®Ò?Gæþ9{³r?Z1`?•'Ýéaƒ?Ô)z‡6"?•'Ýéaƒ?ïßLKˆµ?s.×¼éw¢?pYÚIù?s.×¼éw¢?ï²QæŒô?vËN2îé?ƒk†pýÛ?vËN2îéAGN4FGL J0014.8+6118?åÁo'p@Á¿ôr6~ANÀ9u?èM[ÓÀ;×4ÊâçÁ@ Œ€¨ô?þjbßÉ(Ó?»M•ŸŽü?ÁëvÛÿo·@líԄQ3?ý
ÀN\¯¿ëgT7¹F¿¤^ÞMu¿ã¬Øpnýå¿Ùìý™É?¿ÞRe]Qꮿè
þEjÃAGNbcu3FGL J0014.6+61194C +60.01?ïøZŒ4ù~?N(ÀÒñq?N•Ï)ç"?N(ÀÒñq?ï#Uä§Îª?¡µÝ1¦?›•CnuƯ?¡µÝ1¦?ï«}fˆC?µeÄ"'?… ¦qKû4?µeÄ"'?îb¹öRÏ?Œ}j ?©×äavº?Œ}j ?ï¨Ó½p¨#?֐'0?…Ë f[a?֐'0?èîÎÁ]qº?ˀ)†G\?ÌDÄúŠ9?ˀ)†G\?í©0͟§ó?¤55¥€?²¶y"Lšç?¤55¥€?æA‹œðô?µ"4É+±?Ó|èÆ?µ"4É+±AGN4FGL J0014.9+3212?ã"MäS@À>™»'ˆÛÀ9ض쐷sÀ<^xîÿ&¼@a]Uñy*@}_~ë˜j?¶'+èç	º?Áú
ø' Ï@5µœ.ŸP@¶`˜Ëþ?xî(g¿â–NöÞO¿é¦'™ð×n¿è€åM¸¿ï÷™)1Q²?ï]€C‡>MAGNbcu3C 6?ïýeá'Å
?<p}²åM?4Ðôë1t?<p}²åM?ïò­±uû§?[ƒÞ¾´'²?Z¤výq2?[ƒÞ¾´'²?ïÝ÷ل¯ì?hÿì!?q0™…å?hÿì!?ïõ©\Q±ñ?AÔ -tƛ?T­Gˆ—-?AÔ -tƛ?ïùþÊ\?K;y\¥ã«?K݅•\?K;y\¥ã«?ïË?ú'?'Öe¼Å02?z`éhz?'Öe¼Å02?_Ò3Ð?‹•ø9¸?Œ—'ý´œ
?‹•ø9¸?ïÃb?p궊£M?~@Nò§âé?p궊£MAGN4FGL J0015.2+3537¿©£·­:g-À:­qGÏ¢À;x–z*h‰À<Í@N¤©@!8ÞZh×/?ÿKùƒ<Ú?į	Bsí㿤ä¯þœ
ù?âAªŸ¦N@¾ÌY	‡¿¦XåIpag?§‰\¾$›ô¿é§h5"¿ß¼MΕ¿Óz۞ ç׿Ö±MëE^AGNbllRX J0015.4+3536?ïþָͫ?!ÎÏyìà?/ҒçRN÷?!ÎÏyìà?ïðhÙ­0?b¸ÍlØb?_/æ9gÐ(?b¸ÍlØb?ïäáëå8K?xŽo
»¿³?kç=?xŽo
»¿³?ïø¬}]4?6ŒVGa© ?MN
UÛûj?6ŒVGa© ?ïû"goi´?Bz%2"?A®b	,|Ò?Bz%2"?ïÁYत?Ã؅[TÖ?qS*z¢?Ã؅[TÖ?ïño/ë?mÒU2ƀŸ?]!¡Ùåª5?mÒU2ƀŸ?ïÎP«œ¯?mèàE§?xתºÃè?mèàE§AGN4FGL J0015.6+5551?´(¾ØEæÀ Õ}uv¥À:-ñŽM5=À<@â
K³]@!K'Z°Ð˜?þxòZ%?¹7ʜ›×Œ¿p÷B"ÓÈ?¶6)Ôº­@´€Ǒ?ïþrÎ\¿Ú),VJ¿âôÿý²H¿ÚP*¥Em¿Ûšëÿ!Û¿Ò£'™¾-AGNbll3FGL J0015.7+5552GB6 J0015+5551?ïàšmuF?¬'§]lÙ?oe~×Bé×?¬'§]lÙ?ïñ•'ø\6?d:ÀµA2?\ÔùàŒãJ?d:ÀµA2?ïå"D%|o?s[ç¦O²?j{»Ðä©?s[ç¦O²?ïë^ßD¯Ä?J®RžN?d¡ òIü&?J®RžN?ïø²·UtÚ?EÚ䃧»Š?M5!ù³Û"?EÚ䃧»Š?￉)"ÒØ?½®M¤?€µ«ô"*?½®M¤?ïãÏ8É~?w'àÒ3°.?l0Ç^?w'àÒ3°.?ïƀ±¯ÿ¦?eÓ0ÀowÙ?|¿§2OÆ?eÓ0ÀowÙAGN4FGL J0015.9+2440?î=Avö_ÀB¾µ²ÔÔÀ:Ñó¹À<~µI"ˆÁ@ã&T'Ÿ@ç!éB?¸@ï3t¿±¯Vš@ˆ†?ù'KiŠÞ@ºÄNÎð¿ã|VÝÝ@b¿èÄ(Lýà¿æ	¢–"¿Ú0±CŠÏ¿æÕu³
ƒè¿Í¦ÙÉ	žºAGNbllGB6 J0016+2440?ïþ˜ÖióS?EŒ‡—šY?&r9ôk}?EŒ‡—šY?ïñhÅ]º?]ÄÁ$Géì?].u†"[÷?]ÄÁ$Géì?ïø.—d'ƒ?`M!QLŽz?OE¢û?}?`M!QLŽz?ïùææ©lË?0/èAôŸU?Hddntp«?0/èAôŸU?ïüÓU°";?3Zsr¢6²?9eTBÏY?3Zsr¢6²?ï½Z/ô?Šª
ˆ"\Ë?€¸)kxñ?Šª
ˆ"\Ë?ï몈?ü?v€¸°3Ü ?dUwÄ[‰?v€¸°3Ü ?ïÓ5ÒÓT¯?f‹ÛøÝ›?ve…'œ§?f‹ÛøÝ›AGN4FGL J0016.2-0016¿î+Эï‰ÀNí$ò'Ð)À9oßÏpÀ<&4ú³å@­ã'K°@èƅŠîÜ?³{qæLOº?ǨƒÂAÙi@€8AíH@¢,**uõ?»\$š¿	¿åÿ$£Mw'¿èç6oþ•¿î´w JŽ¿àŠB
ÁŠ¿ï¼=Ó %¥AGNfsrq3FGL J0016.3-0013S3 0013-00?ïûöp»^?B~Ûq?@&@:¥ }?B~Ûq?ïï)¬Tdå?b˜x²›U?`ÖSi¢›¢?b˜x²›U?ï™f{,O?…¹I;ü?‰¦}ëƒÀ@?…¹I;ü?ïùš_+"‡?6¡|m¿Íõ?I–'bªÝ‡?6¡|m¿Íõ?ïü\¾¶£Y?O…eýä
b?=YÌ?O…eýä
b?ï°þ¼\"?‡é‹ÊNe?ƒÀPìBe+?‡é‹ÊNe?îè&zÆ£F?—;yÂ}'Q?¡}˜Qª?—;yÂ}'Q?ïÍõ75\"?m@Ð8?ydQcùè?m@Ð8AGN4FGL J0016.5+1702¿Úª7h™hêÀFƒÑ¼râÀ:³dÀsøöÀ<j³fÊ9@0ù¼‡°@€ºˆ&«?Òç@ìY?Ó¡$'|œ@Ö_Æ	@[Õì¿æžï!‹k¿ä±^ýfr¦¿äì['û¿ëÇ4<G®ë¿ïÿ!Ÿ>õ?ï÷ZtÀœ=AGNfsrq3FGL J0016.5+1713GB6 J0015+1700?ïùÖۙnQ?F¿;§3ª?H¤'ªgÌ0?F¿;§3ª?ïêêL9"v?lR"Ü]?e´$ùl?lR"Ü]?ï"adQ–Ô?ƒhgǶIÀ?‹'¦ä»?ƒhgǶIÀ?ïóD¾ ¹?IǾę?Yv"ލN?IǾę?ï÷¨äÌY?Rí~uŠFo?P®5ã\ËN?Rí~uŠFo?ï…ŽgêÓ?›1æ"åxí?Ž¾œXFÛ4?›1æ"åxí?ï)Rñáю?"}DBfœ?šÕ¡Ç5j7?"}DBfœ?ïˆÔŸÿå(?"_AB'Ú?ÊØåíó?"_AB'ÚAGN4FGL J0017.0-0649?ÞÅÄn.‡ÀQÙŽuyÀ:_ŠªŽÀ<`íjÒò@"†qsµ¯@9^Æ^ô'?·]HZŒ¾j?ŸÐ‡†5}?ægf
öÔ@
63ÍÔ?ïʇ½ùö&¿á#W¾,öÙ¿æ	8æ0¿àéT "¿ç6
]ÑíH¿ÛcS!DAAGNbcu3FGL J0017.2-0643PMN J0017-0650?ïþºD¬NÊ?âp¾ß®«?$[µ—o?é?âp¾ß®«?ïïq³)@I?d4Ôs¹?`ŽL¢…§z?d4Ôs¹?ïð‡NéG,?q;Í,af†?^ñaØ;X¯?q;Í,af†?ïúµÇ
&?1À»fÄ)?E+ÜÔÿ}?1À»fÄ)?ïý¨>h¤?+òqE¹}?2¿FßÖ¯?+òqE¹}?ï°*0L›?'‰'W¹w?ƒúu"jù?'‰'W¹w?ïãuR½g)?|ž‹ÜÅ¥Õ?lŠ­jtNš?|ž‹ÜÅ¥Õ?ïòŸTø—?Ild'šÒ?ZÁV+m²"?Ild'šÒAGN4FGL J0017.5-0514?èç˜8gGÀPª½Qï·À97@´%6À;ۀ
×Y@㵈b—@ÀÓ¢±p?­xm'—ýì?ºé'9Xç@	HdóŸŸ@ÁI©lJ?Ð]÷ÂnÏì¿äŠ&ßè³]¿è-©¼&Œ\¿ér*ŸÔy¿ár\=îx¿ïÿþó…õAGNFSRQ3FGL J0017.6-0512PMN J0017-0512?ïþg 3wã?ò¢ v'|?)…úxøI«?ò¢ v'|?ïð³ÿð?apΦl?^˜Ø)L?apΦl?ïç{fþ'Á?]8R ón?h"™˗?]8R ón?ïÿÖË«?àєùÝ?…9ÐÝ-è?àєùÝ?ïÿ-OÌúx?@¼'›?Ü?V
2·Lç?@¼'›?Ü?ﶊ¾_v³?‰"±kÈP?']PxH}&?‰"±kÈP?ïÈá8û°K?yûr—HÈ?{c€_?yûr—HÈ?ïûÞ£š?3NÆ­ÇØ]?@†»	18?3NÆ­ÇØ]AGN4FGL J0017.8+1455¿áZ3ŸŒÀG•{t¤ÓÀ:£ß\òI^À<‰f1A@s~"?jN@?L¤?Í_,
u?É$Bjۗ?ûqG6w@<¼K <v?ïý?ѧ¿ã/+f¶¿à("` Ò¿àøý!©H
¿æ6""Ý¿è­-]AGNbllGB6 J0017+1450?ïíÑ¿)?©«å•~T?bè.yNnM?©«å•~T?ïìÑÕÓº/?e"zé'9?c.*7D'?e"zé'9?ïâ4Eµtt?pùš<'w?m˺>,óí?pùš<'w?ïâÖÁî!†?MÓ—õÉ?m)>?9Q‰?MÓ—õÉ?ïù‹ÙßÒ0?L¤Uå°¸‹?IЗáÖ—?L¤Uå°¸‹?ï»c¦ÌÁ?'°¤€Xý?'<}ïÐ?'°¤€Xý?¬Zo?‡>ÿ‰P?‡^"Ø6.Þ?‡>ÿ‰P?ï"up˜'?qêG6îO9?Šâ£ëÛox?qêG6îO9AGN4FGL J0018.4+2946?ÌÍfŸ5(ÆÀ@F-¶°`À:[ŒõFhšÀ<RùôMDV@!JË
)úz?ù€ÝàñG?Á*Á_0g&?ºäeb…[?ü}w$#Ë·?ùjž"dÿ?ïx³ÀŒLª¿çHº•"<¿Äê0_ï(í¿ÐQõ–²Y¿álîu"Ó?°m®^kAGNbll3FGL J0018.4+2947RBS 0042?ïý'´Åfs?#§«ÿ0ëR?3jWº	§M?#§«ÿ0ëR?ïÙ]óarG?€(B	Vj?sQjüZ?€(B	Vj?ïðÝTHEƒ?_;O.4õ?^EVèÄK?_;O.4õ?ïlM5'Þê?tEë'Lب?'vYRˌ­?tEë'Lب?ïû%WÓPŸ?8áÔtÚm?Cj \úu«?8áÔtÚm?ï.çv=ÁN?¤Ä.¯Ë9?š#6A?¤Ä.¯Ë9?ï닧¨ú?pü[­ë(4?dtYrÍÃ?pü[­ë(4?íàèflÅ?——%ðbä?°ø¼Êv0^?——%ðbäAGN4FGL J0019.2-5640¿çÇ>­å«ìÀMòÜ­¡À:m'§7À<³[bý%Z@C+xÕ@_±%§Yv?º ZmO?¤-7#`_ð?éÔò5<!ï@O•¿ol¿ÂסçñÁ¿Ó§ŸÁ¦Óê¿åܟ]}ß¿ÜPLßÖë¿ç/§Ã(]¿ï¸uý³¦AGNbcu3FGL J0019.1-5645PMN J0019-5641?ïÿn¦¯_?›¿ïBãù?'+՚-$?›¿ïBãù?ïö•˜,B?WÿÿXSé?RÔüw±{±?WÿÿXSé?ïó|¹äè¢?a(;%X¹?YŒ´ Zz?a(;%X¹?ïÿÇþÜ¿^>ëIPؘn°>üšj[RJ>ëIPؘn°?ïÿ.ÿûV?¢iæO…Õ?ùR¢º{?¢iæO…Õ?ïßiÎêx?pÜ༨ó@?pK¦ð½=?pÜ༨ó@?ïðD"ï™+?mý
ªÒ˜?_w¹éÓë:?mý
ªÒ˜?ïÿ¡"2
>þÒàæ½ÅÐ?Ÿ®™U­>þÒàæ½ÅÐAGN4FGL J0019.3-8152¿í7™VÓ¡RÀA"¿]xÀ9µo`
+ÓÀ<IîsÂ@N1‰9úù@šbÞòi?³f"nd6¶?¥B<Ä	7?ò@‰ƒœ@½×¿â úa§°¿â%\°Úÿ¿á}Gô‹W·¿à\øɪÙ]¿à×~0‡‡¿èï;!>>)AGNbll3FGL J0018.9-8152PMN J0019-8152?ïþOªslÅ?8€ê&|?+]ìC?8€ê&|?ï÷nK«Ó?S¬oƒŸH?Q#iûh	?S¬oƒŸH?ïøÿéUq?EXú<<ü¹?LZ}$£?EXú<<ü¹?ïú¡1qÑ?0TÊ:Sìo?E{9õÇÇ?0TÊ:Sìo?ïüוcæ?/ìêv©?9CTNô?/ìêv©?ïÞ-þýã?~ ÑÓe û?péuÍâÎ?~ ÑÓe û?ïöù[ '?fü'‡Ê?R
I‰GÒ&?fü'‡Ê?ïîq›+r¨?T[%è_`÷?aŽd–´`:?T[%è_`÷AGN4FGL J0019.6+7327?Ô
zí±ô¯@%sõ/ÂekÀ8¬ÿ˜Ñó}À;cgž@–×í<X÷@ÛVà·e\?¬¶áAèœ{?²ûðü¬äO@Å6B²,8@DVÇ?ïÅÒr(;ˆ¿á
/þËLš¿é1rEî¿äõ¹?§4ã¿ï¨ÿ"_{f¿ïÙzé¯AGNfsrqS5 0016+73?ïúå»d?:VñÀ ¶	?Dk¼i©0'?:VñÀ ¶	?ïñtFbú?a¸3kôç?]t³+}?a¸3kôç?ïy24Z¦?ŽÇ6¤›š?ß¹ÀSãD?ŽÇ6¤›š?ïû—Ú–}Ê?3«±ù?A •6o!¸?3«±ù?ïíõ		œ"?`š÷öš'?b
÷ŸûX?`š÷öš'?ï¡ÂÎØPö?"‹(ßêƒ8?‡LM[^"?"‹(ßêƒ8?ï+ÏBrì?"/1ˆóŠû?šŸ†±¢z?"/1ˆóŠû?ïôâ*µ"Ô?PëZöˆ?V;ªqh½?PëZöˆAGN4FGL J0019.6+2022?ïbSßG›ÀDð\|ؙÀ:Z°,ƒÊÀ<|à"&þ@»½•LWò@è"ÿ‰;?¿Ì[㫌?¾[Ó µ'?ü§›4¤L{@*Ò2<h;?ïýròe㊿¥}¯-T¡î¿âë}'üf¿ãٔü{ç¿éì×.OŸ¿Ôܐ¤¨koAGNbll3FGL J0019.4+2021PKS 0017+200?ïôÏî¨?ƒ"©ÂÌò?Vaõd¯Ð½?ƒ"©ÂÌò?ïîÌ1O	?a
ÂÀ—Oá?a3ΜWOw?a
ÂÀ—Oá?ïÚ°&Êç?u2ËsÏ78?r§õÒ}"q?u2ËsÏ78?ïÑ™æ?XˆiPê"Þ?wxqÐ`û?XˆiPê"Þ?ïÄÅ-Šìq?€Ìyp§X"?}i@¹??€Ìyp§X"?ï»à·?ƒ¿«6?ùÒ¤?ƒ¿«6?ïr"x0y?'_{À´ž?'¯pý`kå?'_{À´ž?ïJ;:Ø]?€/©Ùµ?÷?–­øš\Âa?€/©Ùµ?÷AGN4FGL J0020.3+6919?æRÄ}?hB@·¿ŽaÀ:>TÁù44À;£©8s@ºy³ +@ËYÝÁç–?̳*yÑ'O?ÈOÊB®Ñ9?ýóÂî?ãË(²H3˜?ï;ØÞ¨íJ¿ÈʺÂH¿ã¬Y?6vµ¿éZoíÎ¥¿ïÿú¡œGt?î  ¿'ȜAGNbcuTXS 0016+691?ïz¢ßy³Ü?°‹³cf÷?«¤¢~?°‹³cf÷?ãiÕL´IÚ?ÌÈI€Ã?Ù,Uf—lK?ÌÈI€Ã?íÕF–<lî?3š™ñCª?±UËNŠŒ?3š™ñCª?ägߚk?´œEÛ?×1@Ë)è?´œEÛ?ía²µÒèÎ?·µ$ŒÜ…?´òjQÖ­
?·µ$ŒÜ…?·¤§ÙÕG?Î#aâ{¾?íkÓç?Î#aâ{¾?æË@Âì?¶r4dôfé?ÒiÌz'Ë?¶r4dôfé?²oy™û½? 4y»Jí?í¼2Ú~ø? 4y»JíMIXED4FGL J0021.0+0322?ÂÜɾ">«ÀMOÀãŠ~tÀ; a3÷~À<™A<á1ß@ »ÚҞóÌ?û6ìü=?ÐMØ%–¯?€Å'pÛ?õ<¸gºú<@éä.b?àI '–ó¢¿â!3E¨¿äp¹pÏuô¿Ïp-åk*¿Úaj~#Ž¿æ`–
õAGNbcu3FGL J0020.9+03232MASS J00205023+0323578?ïÿ"²é—?ŒZx	œî??"N:?ŒZx	œî?ïï|íø?fG3ïflÖ?`ƒls?fG3ïflÖ?ïù­ŒPí?>mš÷?K™Jn¶èL?>mš÷?ïüÓ	ý¯Ä?!ÑQn1 ?9g°ý͇ã?!ÑQn1 ?ïÿž"J>ÿÏñÄ҄½?zCâCî>ÿÏñÄ҄½?ïÀÉפí?ƒ¼âJj¸Ø?¹ò]ª?ƒ¼âJj¸Ø?ï÷a'Zú¼?W¤dîS¬?Q<ÚçÈ?W¤dîS¬?ïõô(Ë?EùÇf;"?TÄS
w?EùÇf;"AGN4FGL J0021.5-2552¿ÝÜ*¸»GêÀTÌǎŸj"À9¤GOIê/À<WëÃ¹ÿ@¯mŒöH@§¦tso?°/R¾hÛâ?§ùâ&Â?÷$êµë߸@#8Vˆ¢Ñ¿ÞgÃ}î˜O¿ÛyáBz£à¿á$ý°šg¿àl°Ý­ð"¿è=[‹`œ¿ÔÄh¥/úÅAGNbll3FGL J0021.6-2553CRATES J002132.55-255049.3?ïýŒ…|Ê?)y~!ÑÅ?3›×¬ï}?)y~!ÑÅ?ïìuKÜwe?w'>Å"Œ?cŠ´D"Û?w'>Å"Œ?ïèl–èJ"?kªˆØ•Ó?g"h×Å}?kªˆØ•Ó?ïùɎև?7®l#éþ?HÙÅÅڏ•?7®l#éþ?ïñâ¢eßÈ?Yšz­Á(?\:ºÖËX?Yšz­Á(?ï§/¹?™=¤îe?†4:ŸW+ˆ?™=¤îe?ïӃÚ.xþ?~ÇŝIϜ?v>ðLÕ?~ÇŝIϜ?ïñWÑÖªz?Q«
Á`CH?]P\³Ìâ?Q«
Á`CHAGN4FGL J0021.6-0855?&ó="£ÀQžc^J8À:÷ØcÙÄ,À<Ÿ#vý_@Ñ£žU@@DXÍ?Ô5lÉV÷?У–r¬?ûü'¶vI2@£&T'Ÿ?åð ±»ÏO¿áv+ÀÎð¿àvÔb˜P™¿æ.Å_ñ_¿ïÿþÐñ¿îkV斢AGNbllNVSS J002142-090044?ïٌ)TÉA?rņ,'j?s9ëN;n?rņ,'j?ïÞà[R"«?s2Æ­¿?pÒiCŽi?s2Æ­¿?ï8V;Sœ?'ÞPhH?œøõ8•Œˆ?'ÞPhH?ï¬ôµt§?h·!‡ÁC?"ÂÒ°¹L?h·!‡ÁC?ïŸîm'å?…ÄE-b?ˆd°ÝÂ?…ÄE-b?ïk°1'üA?œ G³ã"?'‰ùÌ0Ûð?œ G³ã"?î@Ÿ­Yë? FoŒ?¯ûöHQ? FoŒ?î©@ç.€z?ž7Šœ+?¥kñ«­c?ž7Šœ+AGN4FGL J0021.9-5140?ì³DSI±­ÀP5w ÈÍdÀ9¼•*™1À<i㤦©@ž4E,@m^•—?°F¸ Bj´?ƒ—»W¦Ò?Ñ}0'S×Ã@cː6Äb¿Ætž7ŽÇ¿äÑå©és¿ÞaOÛàf¿àLJžDy,¿Þá\ü°?M¿áñŸ,ݯAGNbll3FGL J0022.1-51411RXS J002159.2-514028?ïþ¤2RŽ?C¼v`»Ó?%¼ÛÞ·9[?C¼v`»Ó?ï÷¶âÍ®?SÄˌˆ÷y?P':pö?SÄˌˆ÷y?ïöï€Uûµ?[‰ûŠ†…?R ÿPf0?[‰ûŠ†…?ïÿ=&ÉdÛ?
þKxg?['*yy#?
þKxg?ïþC˜õ?!
'f?+ÎZ?yÉ{?!
'f?ïۆ`N@Í?]÷Yε~?r<Ïø|F?]÷Yε~?ïø¹:Qh0?cqC_h?Mdvg?cqC_h?ïþ¾ ƒûo?™gÉS¢À?$øÅ?™gÉS¢ÀAGN4FGL J0022.0+0006?íÒ»ÀÀNí؃º4DÀ;/…(ÉÀ<~CvwU¢@#zISž?ù;ë2éaX?À2AƞàU¿®p——¶Àq?ï"{[>@×ä"Sçß¿ï&%z
?ïþC¢|l¿äVÇ¡Р¿ãȑ¿/«>¿à@óæJ?àâÙ,,¯AGNbllRX J0022.0+0006?ïÿ¹m'(?-8_N°Ý?ÈË
ï|±?-8_N°Ý?ïì¤ó·>½?fÙîpýî?c[0«?fÙîpýî?ïè"Êï@Ú?iÎÜÖâ?g{5~Ö(?iÎÜÖâ?ïõ3£E•?EŒ'tR:?Uјõíõí?EŒ'tR:?ïþjR†?%ë¿Õ¯?)ZÞYÔ³?%ë¿Õ¯?ï±é?°UY?ˆ4À™;9?ƒ…°*ùÂ?ˆ4À™;9?ïèïÀAÏ?rQ¯æ†3?gæ…aU?rQ¯æ†3?ïÀÓsžÌù?xáÁçn¡7?–F@g·g?xáÁçn¡7AGN4FGL J0022.1-1854?íuU¼
ü‡ÀS×õY³Ð}À9Ÿ‡mG+8À<æ¾æZ=@2ý2Ys?üI(gþ?´Y¢ž%•?ºë¬ "ÚÆ@¼uf´iÿ@#¤^º?î÷*¾ðk8¿Ýµ‡9᣿ևî@¿ØM´ÿ%ºz¿ç‹^Öw¿Òl"h	ԕAGNbll3FGL J0022.1-18551RXS J002209.2-185333?ïý1?NZ½?7Hš3ë?6v…§o8?7Hš3ë?ïåA•C ?t£ë`+?j¾j–o@F?t£ë`+?ïèǤÄÅí?mçû?9›i?g8[`Uژ?mçû?9›i?ïÎY$'>?`8‹wÅñÖ?xÓm¾ˆ.?`8‹wÅñÖ?ï÷žs·Ìy?JÂ
	[?PÃô-í?JÂ
	[?ïz†áR8?ž"ZH(–U?¯#Ò>½?ž"ZH(–U?ïÊ)L:Ò?'_¶s]‡?zðko0*½?'_¶s]‡?ïZhý֖5?'ߐ`@K?"²àJT£K?'ߐ`@KAGN4FGL J0022.5+0608¿ïòü³‰ºÀLl
oTLÀ8Ÿ6}jŽêÀ;¢OYÚg@û£è§ô¦@|\qðÞ?¤ "ˆÞ`s?ªMúY
°@8ÑØ¥H@F_Á܃ϿÃGw£O¥Û¿Ý¸¼yBŒ¿ã7õfI
¿á0[è^"Ë¿ã–#£Â¿ê
©ÂÉnAGNbll3FGL J0022.5+0608PKS 0019+058?ïúÍíÃg?kTã{Ì¿`?D˳c&?kTã{Ì¿`?ïò¡¼äÞ?`@¾ûj§c?[¼Þ,B—?`@¾ûj§c?ïò=åhÏø?a?MÇ­Ùæ?["4Öj/?a?MÇ­Ùæ?ïù՝Œ
?4vˆ+þ:?H©ˆ¡³<{?4vˆ+þ:?ïý¡ë;'•?+g4•6+É?2𥪁è?+g4•6+É?ï½ë{
½X?†-NSä?€…!-l?†-NSä?ïåo±úʝ?sӖàº?jN*Q*Ÿ?sӖàº?ïïä›íÔ&?OŠüË?`d<Çñ?OŠüËAGN4FGL J0023.7-6820?ÝÈoY÷eÀHJ"‹ë[-À9òóú8?âÀ<' Í|@þ¥aùÅ@›2öÍ?µp(.mQ?µ áL
Ł?ø3)ø÷Î@Gs\/¿Ðj@ºˆ'¿ç3®eÙ¿éès€¿åÀþŠÓ¿ïÿþÐñ?äñ*å†×öAGNfsrq3FGL J0021.6-6835PKS 0021-686?îãsâ¥?Â,µ­Bæ&?¡Çϝ¼³?Â,µ­Bæ&?ïöx´¿]?Sö»$°ã?S–H9Ö??Sö»$°ã?ï¬ÊS ?‡«sd:b?"û
rœd+?‡«sd:b?ïý	à á"?*péï°1?7°üZþÒD?*péï°1?ïû¦³á?PqºN8Pã?AgN"õC?PqºN8Pã?ïՎsº{«?€¦YÁH|t?u8ÆÔn?€¦YÁH|t?ï¯ÊŸÁ˜?ˆ
 Ö¸~¤?"
X*}õ×?ˆ
 Ö¸~¤?ïês{D;f?]›Öã	¥Ê?eŒ"Ó!ò6?]›Öã	¥ÊAGN4FGL J0023.7+4457¿u…º1ô'²À1¥3ã\[KÀ9¸AûMÀ<PZUÖ@ôrÏ«Nx@aE•6?²»®·Ë?²ƒ:\9â?þ/ˆØ6@\¼üË@?ïÅJŒì-¿ã¡Îò@û¿åÑ瞊D<¿æ‹¡>(¯¢¿é8}¿H€¿æ_AtyAGNfsrq3FGL J0023.5+4454B3 0020+446?ïþ|KZÒ?OwbZ?(;OýÎóå?OwbZ?ïõénC) ?W-¹Ýkx?T-#7_½?W-¹Ýkx?ïîÈ-UÏ?MZŸí	ãZ?aå7¿la‡?MZŸí	ãZ?ïüìåØ?(sI)^?;ð™7€Eý?(sI)^?ïýíôŒ?%`Ó»~<?0'à›"Æ^?%`Ó»~<?ïÉåfC"a?‡¥¿5Ã,ü?{
Lݾã†?‡¥¿5Ã,ü?ïßßj¢úÛ?sŸêïe¿?pJ¥"–?sŸêïe¿?ïø7ŠÁö–??zwҝvy?O!Õ¯ãí??zwҝvyAGN4FGL J0023.9+1603?ïGDRÀG%ƟŒ!âÀ:"¬ñe2ŠÀ<s
=Ö$@É­"£:­?ÿPœÐ…¿?ǸÖöœT	?ÀxxšE'?øZÁ¶%@S$彉Ž?ïâHZ⥿ã#˜ ö/G¿àsÉøÜö¿Õƒ
¼õ¿éÕ	ÖB—¿æòçHy–AGNbll87GB 002122.5+154553?ïöïåD©?LfÂ
ËU?R 5;½ý?LfÂ
ËU?ïé/Pûp#?jSac‹­U?fЯ6
<h?jSac‹­U?ïÞà?gÁR?jŸ™òˆ?pà:ñK:?jŸ™òˆ?ï¶R!yÊ?b_‡6¯l?'kw´úÊ?b_‡6¯l?ïÆD‡ïM*?x³õ2Ù?|Ý»ûJæè?x³õ2Ù?ï«­wÆ­?‰ß²ž‹+?…¿¥}ðŸ?‰ß²ž‹+?ï'홲)o?‹Þe¾…=??‹"™‰&Ðf?‹Þe¾…=??îîà
õj?†•÷Žòj¤?¡´^b?†•÷Žòj¤AGN4FGL J0024.4+4647?Ôì%|*6ÏÀ/¥Þ7X[âÀ:þŠBäÀ<`;`(^Ä@½$Ö¤@Œ…=Â?Ã4øŤ"¿«Á}ä1m?æÀPQ_@	ïùÜOv¶¿àhˆ•â¿éiáyð‡¿ëEM|Š•¿ÊÐԙI聿ïÝˍ1¬J?î'¢ PØ`AGNbcuB3 0021+464?ïþÛÃ	Õl?â
èÆUx?"CÑÅýXÍ?â
èÆUx?ïõÑ¿a¡?WðÕN~MÆ?T\@ nÌ?WðÕN~MÆ?ïëˆÑAÉ?aõW[4È?dñwKšîè?aõW[4È?ïþýÆÇõ?W‡Ì"!? #œ"äÈ?W‡Ì"!?ïÿ=ˆ™?/¸€ùÔ?øJÒ¸?/¸€ùÔ?ïÎG%®eY?~²ãç®k?xÜmÑÞ?~²ãç®k?ïê±"¼p?kK@©ì?eNÝ`è?kK@©ì?ïö¨âÀ]?Jþ"T'6®?RÞ®`úæk?Jþ"T'6®AGN4FGL J0024.7+0349¿ï75"ØR£ÀM0i@5z5À:ß[†8"ÅÀ<t{i,êD@Ç-õ±q@	þCg]Ý?ÈcŸŒ¢»?¼Ù©¿Š¯?òî^íÌ!@ê0ðã­d?Ä"SçÞ¡?ï–7D9ë´¿é yó$÷¿áß-WQ­¿æ¤õ8%á¿ïóÉü7ôcAGNfsrq3FGL J0024.4+0350GB6 J0024+0349?ïÿ?Gµî†?ŠÜy¡™?$€ù?ŠÜy¡™?ïðu‰w–?e;(ø­2v?_ínI1?e;(ø­2v?ïèàÖ¼\4?gþ
ž‹Õ?g)KâÜK?gþ
ž‹Õ?ïÿ!Ø0Çã?8F¥À?Äñ]/f.?8F¥À?ïÿiQ? õ¡™(s"?'Õ~¥ä? õ¡™(s"?I
Õ֌?†ì#š²ö?€Õ¼–ÿ?†ì#š²ö?ïÒ{¿WÝü?~v !ÄZ?v t]U·?~v !ÄZ?ïýxUžo?+ƒPLÌY?4=Rƒ-¡©?+ƒPLÌYAGN4FGL J0025.2-2231?ïåCûq>ËÀTŸ!BoçÀ;'›]:À<®ÑOŒÊ@u*ÑsP@#5ߵݝ?Âí'úÆ°(¿¢‹ìCíþ?ß¡J½éZ!@àë¡y6ù?ïÿÃF1=¿ásÁ}ä1m¿í§À8iÓÙ?°‡Ãs¢º¿ïÿØþ3w&?ïþ7ޓž®AGNfsrqPMN J0025-2228?ïóNéi‡û?[&|­ƒèú?Yb-/¯¹J?[&|­ƒèú?ïé¿Y$?tÊ
[Ýt?fô@ÛǤ_?tÊ
[Ýt?ïyµ4n‹h?‰ø'θû®?ÉYr."?‰ø'θû®?ïú~Ž{Xf?7ÑÞ> '?FÆXüÎ:?7ÑÞ> '?ïÑÛ§±	x?}CãÃ]&?w,%k€?}CãÃ]&?ï…Ô'p)«?˜+»€ÛBí?ŽŠßRljR?˜+»€ÛBí?ïoŠ§yŠ?'ÑËÒ5s?'¼ËÎÉ?'ÑËÒ5s?ïÒcÝu£?q|³:š§¬?vÎEw®b?q|³:š§¬AGN4FGL J0025.7-4801?ëґTH#ÀQ!©æî·À:aŠ ÒHÀ<"P/Ã<*@H¹»øê?ÿm…/J?ÍiKH'áñ?Ê3E½#Œw?ÿ±¦Ö˜þ@I";ø¿çqCĐ¿Âw&gÈþ¿äZ1®
j¿ßýäqÚ
¿ë	^î¢àj¿ïÿÀ¿ù)ÍAGNbcuSUMSS J002545-480356?ïùâØãíŒ?D9¯™Ñ?Ht|'µ1?D9¯™Ñ?ïö%Ì?V)"ëc9?SµÜO¢¸?V)"ëc9?ﶆŒ&?z¯ý4¦×A?'^\ñapw?z¯ý4¦×A?ïÿvRl´^?ÀþÛ̟?5·yT±?ÀþÛ̟?ïüoÌ
Á?=e©ÓÜfø?<‡?ùs'9?=e©ÓÜfø?ïÞ¦'Ý·?rãۗû?p¬ì{¡ˆ'?rãۗû?ï-ü'6?•[…DŸƒ?:@rÕÃ=?•[…DŸƒ?ïþòkí¹×?ÊÎ.ÿÆ? Ù>#µŸ?ÊÎ.ÿÆAGN4FGL J0026.6-4600¿È&	Ê.6õÀQžÏ€Ü3rÀ:Îùn‡QÀ<µG› @헗‹ÍS?þë׉¿1?Á!q)búÌ?†óxæ¤Aò?É»g_4Ã×@üe+Rê?ï÷´×ãD¿ã§E‰w§¿Þ€§ZL|°¿×ÂC[õIC¿æ›ëþì.½?®¬ù$AGNbll3FGL J0026.7-46031RXS J002636.3-460101?ïþ‹›Õ0?õo(ê¼?'FAȗFû?õo(ê¼?ïöy½lmÎ?V?éϏé?S…Vô?V?éϏé?ïðx"îŸ?rhIq¹WÜ?_ןëÊ?rhIq¹WÜ?ïý–4þB?"¾Ð³¼`?3OM9÷2?"¾Ð³¼`?ïþXüÒµ? Rzã^.?*~Ÿ˜æ.0? Rzã^.?ïÜ¥3
¦?u;nß:qn?q­fp›uF?u;nß:qn?ïõ	3šr?jf_ëƒe?UíÛTë"?jf_ëƒe?ïú>³L¦ª?73SSE¨5?G25©Êª?73SSE¨5AGN4FGL J0028.1+7505¿Ûø¹"ñké@(–G™ÅXÀ:Üéä4È_À<¶‡•@y56Ì?ü½3«(?ɯ_Éî?Û'‡W@
Ä_@wÏ@d
+' *¿åJ¬–Ì_À¿ê,9¿iaî¿­ª±ÄޖϿÚÛ5{Ù¿åøšá"¿ïÿGuܦAGNbcu3FGL J0028.6+7507GB6 J0028+7506?ï]ΛE–?™aIÌÙ?"F'¥¸C?™aIÌÙ?ïu×Ù¬jh?—|í˜G«?'EÊr³?—|í˜G«?î–ï'ÀŽP?™j•ã7?¦'
'?M?™j•ã7?ï
žØ·€y?{/†Ù`?žL$â0¸å?{/†Ù`?îûTb`zó? l½äÊ¿? J¹ÚÔ7Õ? l½äÊ¿?ìäVØÔÚ?À[Sßa`(?¸ÝI9r5?À[Sßa`(?è'ñÌWÿ=?·Œšô¿?Í´8Π
?·Œšô¿?ë ܶq8?§g¤vcÖá?Ã|&;ˆ?§g¤vcÖáAGN4FGL J0028.4+2001¿éè5fZPÀEAÑöy}À9‰þçÒÑÀ<B_•'Í@¹T
¬ç@Þ=½Ð°‡?±ÜæàÊ/º?¼l¡
ž¿@Ôøš°ðÎ@•wO>'?ïíKþSý¿áH€Âˆ%S¿ç{š—¿ãðgȖݿîÊˆNî{¿ÉxN…ÊðAGNfsrq3FGL J0028.8+1951TXS 0025+197?ïý<Ð&.Ï?,œdØ*+ˆ?6}l~–ƒ?,œdØ*+ˆ?ïò€`7£/?^¢²?7?Zÿ?àp²?^¢²?7?ïßû^–Ên?mÔóª	¾?pP¬[¹G?mÔóª	¾?ïøî É=?;<‹44'?O€GÓ·'±?;<‹44'?ïý"ž‹?1{¾YòÜ?7Ãàg?1{¾YòÜ?ïËÆCŠˆ?6Áô³Æî?zÞ0mI?6Áô³Æî?ïÄhHØzÅ?€;š"‹?}Ëۭߥƒ?€;š"‹?ïçKÑd·?Zëņízƒ?h´.›Hñ6?ZëņízƒAGN4FGL J0028.8-0112¿ï46φ!ÀOÁàâiÀ;f؁5õ…À<œÉÄÐo@ 	{XæËü@ Ï[†I?ÏèEú
G­?wS¨ÀöLD?£É<quc@ù'#V?ïþž¹"¿èœ³sӌ¿é!P|ð§¿ÑÒ¸~âH¿â³'ÒÓø¿Üj¨ À€AGNbllPKS 0026-014?ïþÚ!ãÄO?£©oñ?"]ßïVºe?£©oñ?ïðÈG,|?cSöùÑO¯?^oqïZè?cSöùÑO¯?ïõÀ¥Í?^ºª7'ík?UÈ~Õb8€?^ºª7'ík?ïýÙÆ@§Ì?˛Œñt?11ÎÛ"C?˛Œñt?ïÿtÓ¢»?'~8"v§?eŽ
9?'~8"v§?ïÆ>%³ ‡?éCº7Én?|àí'Ä¥?éCº7Én?ïö`Â7{?`×ipò=?S>{–Di­?`×ipò=?ïö\lL`?G(œžŠ-ç?SG'?_Às?G(œžŠ-çAGN4FGL J0028.9+3553?‡É¹¬ewtÀ:ÁòfºI=À:…ðÍ]…À<x4Ô#&@Ržý0ÂÁ@"*ú?Àv\¨¢v?"ib''ž?ÅAÓ_
+¸@ô1ÿ¬s¿¶Là®V4¿âcK^£#†¿è𠬳R¿ÒýcÃHê¿ëGÝ^ëGâ¿ïÿÐÀL`×AGNbcuGB6 J0028+3550?ïû—A
ó_?5ø!¿¾€?A¢ûôI*?5ø!¿¾€?ïó‰.^Úx?_
#™o?Xí¢ÙÖïê?_
#™o?ïëoxïç?c6­'ÿã?dæMV©<?c6­'ÿã?ïú8J´Ñ?/u›6+-?Gí×¼¾¨?/u›6+-?ïö­N†B?M·¿ÕY—ƒ?R¥ûµj?M·¿ÕY—ƒ?ïÓ}ŒâjÞ?€×Mí¾Eá?vA9ª÷]?€×Mí¾Eá?ïët›ïpw?sٟ—­)È?d‹cΗ	j?sٟ—­)È?ïìä.ü?R¡&ðËÔ?cììË`?R¡&ðËÔAGN4FGL J0029.0-7044¿ä ÖWm­¶ÀG"—Oß;À9ñÇ9åÔÜÀ<|"ÿ‰;@jÆm¸@k›v¬?·»Z‰Ž^¨?¢ÿËÒ¦Ö?èfÓP0š@‰UC©M?ïÏ8''
¿æ_>ߎÆW¿âPÿÌÔY‰¿Û+ÝÿO+¿ë‹Ÿps/£¿äýÛb'ÆAGNbll3FGL J0029.1-7045PKS 0026-710?ïûbÉÆ?6²*͒Ìl?BtÛ9\"}?6²*͒Ìl?ï÷BF	®?UœÑÉ€?Q{sÄíã!?UœÑÉ€?"]g?‰î`ÒE
5?Š»Zè¦??‰î`ÒE
5?ïý"ÊÞÇ1?$8¾"×âø?3a¨­jŽÕ?$8¾"×âø?ïõ°¶d?JPàgO?TŸáðû?JPàgO?ïÛèxú½¡?€,ÀUÚ¢Ú?rÃbTÛ½?€,ÀUÚ¢Ú?ï¶YŠN¼À?…ºtÙ¼a?'iy·IØ?…ºtÙ¼a?ïûÕùÇ+Î?8 °0ó?@¨ÂT‡ñ?8 °0óAGN4FGL J0029.4+2051¿ïnŽ#LhíÀDÛG"#À;e‰˜š–À<¹"²²o@"töL"?öó•Þùõû?Ö"ˆô'?Óq"€¥×À@' ùà+N?ÿjDŒ¡äl¿ïß|7‰¿í8Ô'4!p?ìpéý_;Ð?ӎ˜ßŠi¦¿àXºvˆóY¿n(™) ÏAGNbcuNVSS J002928+205332?ïü}‡rÙ?/g¹aÖ
?;Ӟ2?/g¹aÖ
?ïí›ڈ«?c˜¨ÇK»æ?bdûù|U?c˜¨ÇK»æ?ïÏäJ܋ö?q¢qʔ®Ž?x
Úo]í?q¢qʔ®Ž?ï柗Ɨ?Z¶klvª
?iø`¤²ˆÈ?Z¶klvª
?ïý(jŠëß?1+úõÌ×?6¼¬aXÐ{?1+úõÌ×?/ÛTÏæ?'î^‹ßC]?€Ü	!Ý
‹?'î^‹ßC]?ïæd—ž©?n`Êàg ?i›h$!_†?n`Êàg ?﵉ú•2?y¹-y†ò?'fº!¹?y¹-y†òAGN4FGL J0030.2-1647¿ãN¢»^îÖÀS¤5"_õÀ:YÚ´¢À<\ãW±˜@ ŠÞOV)'?úB`²È>É?ÁÚ­àùT•?Á+"V´l¯@—ãÓs@g[¢¾Š?ïÛÛÞb¡`¿½ˆGù黿À´±øàüÛ¿Òµ(kY¿Þ×e­ê¿ÖN²?­¿ìAGNbll3FGL J0030.2-16462MASS J00302045-1647130?ïÿ2jóÂ?
ц[eZ?²Å+¦?
ц[eZ?ïïjwÜÊ?e½»¹‰a?`ÿ•©už?e½»¹‰a?ïöêüsêš?B±Ò×ìw?R*ÿmœÝ?B±Ò×ìw?ïûe}¢?*ÊÓ1T@C?BjkŸÌý?*ÊÓ1T@C?ïþ*ÆZË[?#ð²íóŠ?-S—Ê"Ð?#ð²íóŠ?ïµU®'Ú?ŠW=Qå½ï?'ª"…‰õh?ŠW=Qå½ï?ïójÝ]WŽ?a"žÍÉî"?Y*E'T•?a"žÍÉî"?ï÷{ú¢H?Beêå«q?Q
<þ8Ú?Beêå«qAGN4FGL J0030.3-4224¿ïû}(8ÀR‡öý!ÿ.À8â'­ÄÊÀ<1˜F³B¸@¾èÈUï¡@å|Æúü?£Hl!ޙu?ªCŽJ0%@?ÞèXD@u9ÉOiË¿×&F{9‡5¿äúNEq¿ç3SÿÜn«¿æœ}ώž¿î":귙_?ÆNÖgUN¼AGNfsrq3FGL J0030.3-4223PKS 0027-426?ïýú†Êµ?%6 u®?0+Í;]˜¸?%6 u®?ïõìÙæ?X›íjQ܄?T&LWŠî?X›íjQ܄?ïÁEÌà:?ƒkÞ9g?~ÝÒ²ó?ƒkÞ9g?ïý=KÕ?+› @7?6v"€[?+› @7?ïþm+c?(3ÉB±sK?.>ʧ…8R?(3ÉB±sK?ïÜ×qý…?ut쯡ÞÚ?qðL€²?ut쯡ÞÚ?ïÃÇv\äÄ?"ó2åJ?~D¶¾V?"ó2åJ?ïô–Ç?R6OŒ¿?V ð4`ÒÏ?R6OŒ¿AGN4FGL J0030.6-0212¿æ"õ»áöˆÀP%‹'¢À8Éõª;¨MÀ;ã{ÕctD@—ä´,@e…—"?§$ñž_Éa?Àpü}êg@°y=Ùc@XÕ
¥?²р)ŸÐ¿àZÖk­Î¿æ¯Ãzm"¿äqêÉ7¿ì"C çU¿ïÿ%¯¼ñAGNbcu3FGL J0030.7-0209PKS B0027-024?ïñ3µþÃÚ?X›Hÿ?]˜"­Aý1?X›Hÿ?ïï*þ~ð?búõ£1}9?`Õ%7Ð?búõ£1}9?ï˜|G=,?‡çoÛ¯?‰àî-IÙ ?‡çoÛ¯?ïÿÎf¼?²Oˆß+	?,"X·?²Oˆß+	?ïó '$c?R5Œ3"~ë?Yß¾UŠè?R5Œ3"~ë?ï­@¼¢vý?Ž¹ëß祤?"¯ÐÚÑÜÒ?Ž¹ëß祤?ï´Y.ø'?…E{¸œ¹ì?'é½ïqÊ?…E{¸œ¹ì?ïýp·´H?-Û¿Íø["?4zCk!Ož?-Û¿Íø["AGN4FGL J0031.3+0726?Ýtª7eÀKŠýq?À:è7Åi+=À<•(+˜4?@ €³¾"æ?ý\\ø(›*?Ç/–Æ€'q?¶/O"ýÛã?ðœcÈý4t@…¼¿äqN õC¿ìàß8³¦?ãE—Ne¾¡¿èüᛐë?™<ä"Eí¿ãÕàòž™AGNbll3FGL J0031.3+0724NVSS J003119+072456?ïÿAGâ±?0ˆŠ4?×	¨J5?0ˆŠ4?ïñnRz?`›©hírë?]#ÿ,Q1î?`›©hírë?ïó»ÿJ"Ž?W¯ªbù¤8?Xˆ‡7Ãñ?W¯ªbù¤8?ïýŸvŽÞ?" ôµtèÂ?3IÍ*8|?" ôµtèÂ?ïþâ†;]?"'Çå,Ë?!ß¹;ç¾É?"'Çå,Ë?ïÃpc{‹£?…hoayÒ?~GÎCš›?…hoayÒ?ïóعâ[Í?cðj6¤?XNŒjq?cðj6¤?ïøݐ®'_?D,•Ìð?L‰½Ýß?D,•ÌðAGN4FGL J0032.3-5522?ç!¢œÍ€§ÀNÆE܃#6À:MŽz¦^À<|R¢dCv@(W·L@ó•$Ý?¹JÔ»?Ś"U•]Ë@	Ëþp³Ç@¶|‰"g¿Ç
G_ɔ¿ÔÍ×ú'xë¿ä¯JÛÆdÔ¿æ+|_÷âO¿âVlSq¿ïÿòÿf}
AGNbcu3FGL J0032.3-5522SUMSS J003210-552228?ïûˆ¾nÔä?A5‰¿ÓàR?A݇Ž¾ú?A5‰¿ÓàR?ïö!à®	?W-ˆn
	?Só¼™Yø?W-ˆn
	?ïتÜÀ"a?o9ô½D?sª'¦•‡e?o9ô½D?ïÿëá}>Õö¬zc?>äðO;ËxI>Õö¬zc??ïýƒ¼É±?3ÿc1§´ß?7ƒá|w?3ÿc1§´ß?ïÛNeÔC?uTÂE{‡?rXÍuåòz?uTÂE{‡?ïW"RÕm?Ÿd'Yg?•
•·.Lf?Ÿd'Yg?ïÿÑ«r£Ð>ñïáW<›z>÷*L͎˜†>ñïáW<›zAGN4FGL J0032.4-2849¿í6S›ðÀU^c^J8À:ã¹L½GõÀ<¿×ç³ @»ï¶ÝÍ@mnÛí÷?Äy™ßd©ù?·JÌå¤?îè³³ S]@-½@gÏ¿åÜȝ¾|¿Ñø%?–¿åÔdcP¿æ#JóCY¿é¥va†,Õ¿µËÍô?,'AGNbll3FGL J0032.3-2852PMN J0032-2849?ïúþl	Ç?B›p~V=î?DP7ÿz×?B›p~V=î?ïą̊d¸'?v®[	v?j3W×ÀŽV?v®[	v?ïÒgüò*?sXæ}¥U»?vÌf­—&?sXæ}¥U»?ïøÒOâ/?7Ã8£a?L·ªÿ°o?7Ã8£a?ïîØ[²i…?]\­vaƒm?a'¤<âè?]\­vaƒm?ïtÔû€¦?š(XÑ·Ê?'nEbG¹K?š(XÑ·Ê?)1Ó?†š$'6Æ?‡Øu©M·[?†š$'6Æ?ïØté¿e?e®5Á°Ÿ?sŋÓ1¬?e®5Á°ŸAGN4FGL J0033.3-2040?½XDq–g­ÀT•zxl"hÀ;ʦ—®ÞÀ<æMú^Ö@!?Ô¶P3Ÿ?ûØdàTi?υ˜…ÈVp?µ·@Hšx'?åD¸aý–?ø‹
ë@€N?Ç#v|´¬¿ïþµbLü2?ï˟`Xy¿ÄðáxÚ¿ë_÷auæ·¿x'Úì'ä~AGNbllRBS 0075?ïûÇâg^?6;`v'¬;?@àwdÙîj?6;`v'¬;?ïæýP*îI?m_õÅÔ´ò?i¯ÁÓçJ?m_õÅÔ´ò?ï¦pÆÖW?'XC‰|Ëð?†cÎFú"N?'XC‰|Ëð?ïÕì•-èà?dLAjí´?u	µ€hç¾?dLAjí´?ïûarHQ?<«¹ohC™?Bz7boœR?<«¹ohC™?ï'{¥	\?•J©—I¥i?‹{a'ë´ø?•J©—I¥i?ïÖÙÙ$Éä?z·âl2¹?t"[
*(?z·âl2¹?ï–þä÷æ×?'>O"Rgb?Š@FÏĺ4?'>O"RgbAGN4FGL J0033.5-1921?ïð[DÐïÀTMäÍt'yÀ8<Sz
ˆÀ;Pv'¤‰¸@p0ÙÒá?ùꍺß?¢•¾î'Å??²‹À"¦£@|¿ôw5Â@:ÁmH,ê?ãC0×?³´¬š}DN¿ÙՐàãZ-¿Ô!&€È<o¿ÝŒ=ZÔaí¿ÝV"Š‹ßAGNbll3FGL J0033.6-1921KUV 00311-1938?ïæNY{I?‰˜¤+aæL?i±¦ÁFÎ?‰˜¤+aæL?ïá–dþ(Ý?ˆýð±-‰ü?nišú÷ëO?ˆýð±-‰ü?ï¾¹­eÝ?"Ù,ˆ›±?€Q½%$¨²?"Ù,ˆ›±?ï덼/Šv?QñËöÂK`?drC·?QñËöÂK`?ïí5}e[y?hç¹»?bʂ¥£Fx?hç¹»?ï'þ;sZ?•ŒÈVĨ~?‹@q#©s?•ŒÈVĨ~?ïÌI™þ.?"9_Š8¯r?yÛ3S$ÑW?"9_Š8¯r?ïÅ'Müž?p‡Ã°ÿÉÈ?}l7ÚaˆÐ?p‡Ã°ÿÉÈAGN4FGL J0033.9+3858?ïè³æªwÀ7ÆÛ3—ÝÀ:h9Y½áwÀ<v[€YW@>|›Üë@Q«›úœê?Àj˜^D?©þñÀª³%?æíb6V@
¿Î÷õD?ïü¼ž×F"¿ãÆC{Ó¿å+$ p¸Ð¿çÕ)ÈPfJ¿åŽmìl¥¿èޝ´K!AGNbcuMG3 J003408+3901?ïþö]Èe½?†]L@[I? š&?ìýõ?†]L@[I?ïôÃÚ=H?YÂÅ
®S>?VxK|¾_&?YÂÅ
®S>?ïõ>¤;?B CñýU?U'·ÜL
?B CñýU?ïû
E[ÝT?+3+&*[-?CÖê/<&½?+3+&*[-?ïþÄÁ<? ¸€	µå?#³î'é? ¸€	µå?ïÓj³?óN·¸.€?v@J˜¶Œó?óN·¸.€?ïð{œÈ<?eÀéY=f?_ÆFLŸÔ?eÀéY=f?ïðD™+?I‡ž®pR[?_vÎ)¢r}?I‡ž®pR[AGN4FGL J0034.0-4116¿ÑOɹ>rÀRÚu%F
¦À:}à{Ö:À<|Ïç/O@èOiõ'@"s9³õ?»ö•Žòø?"p?Ùð??Õò,'¿ãZ@‡æ¦'¦`?åÉTb,ðÏ¿åyêPì¿é'Ò§®/¿çD-÷Š¹¿ßg49eý¿ÜÙü€n¥OAGNbcuPKS 0031-415?ïþÐ!eÑ?¦B1y?"ýé?ÿÅê?¦B1y?ï÷ª¹|ð?TZ?e•`ó?PªŠÕ?TZ?e•`ó?ïî!ÔN?e"CúH[?aÞê2řb?e"CúH[?ïÿÂ;Š€Þ>íÉÖJQÑ>þâZoR»=>íÉÖJQÑ?ïþ2	‰ãæ?%8ô,Í?,ße9P?%8ô,Í?ïÙUä/ŒW?tûÊæc?sU
Ð,?tûÊæc?ïêée^Ôw?i÷Í_Ñm7?eš–,ÉU?i÷Í_Ñm7?ïÿù°8J?£ˆ[ôæ?ÀÇÜ
Ý?£ˆ[ôæAGN4FGL J0035.0-5728?ê˜(ÒuòåÀMÂDú<À:Ö-Ç©­À<—üñý@™ƒlÜw:@={ 1ί?Æ¢*cÖ¿?²PßkŠè|?é5Ü@W@"½a4?ïèËùo˜¿åªqѺ¨¿èMŒæ,ð#¿æ×ÔÓ+‹Ÿ¿ïþÓ°Üá?èÁ'e±ÍAGNbcuPMN J0035-5726?ïý§^Ô!?3ÿ
ï,?7ÒÄÁçÃ?3ÿ
ï,?ïïӞ3m|?m[º
/]V?`,b‹º?m[º
/]V?ïٗhte?pE7*_?s4L
£ÅU?pE7*_?ïùYÀMÒ?6Ñ /=G?J™ø‡|®9?6Ñ /=G?ïýüñ"çº?4[§îüÒÞ?0tN@ÇV?4[§îüÒÞ?ïÃç	}Æï?'F×đXÇ?~{3^"?'F×đXÇ?ïÐ$êu'?`—FçpÁ?wíŠïG?`—FçpÁ?ïÈУhqÑ?në
ç{V?{—®e43x?në
ç{VAGN4FGL J0035.2+1514¿ãŒ7ÐjªÝÀG¹‰a=1ºÀ90õ üÐÀ;¾mÏç3€@Jz'ýö»?û{fX#­"?®Œæ>.û?´Àû³?2@	QÁ
{é…@
ë±îO(‡?ÚqžÞ|øy¿Ø‹MÜ+åa¿Ù8PϞ¹¿Ø(.½'¬î¿ßqÂeؿṈý•¨AGNbll3FGL J0035.2+1513RX J0035.2+1515?ïþa•y×æ?ÇKۂ¡?)æ¥0x?×?ÇKۂ¡?ïñd#ô"?`pE7ĞÊ?]7·Ì¿qª?`pE7ĞÊ?ïðÁŸ®AØ?Q¼0‡ÆL?^|Àí³Þ¨?Q¼0‡ÆL?ïðv}¾Od?AÑ•as?_Ah¸?AÑ•as?ïýFè¥N?*·å0<r?5ȼ‡ÞBÚ?*·å0<r?ト#zÎ?…%H¨ª?€^÷ÉVp?…%H¨ª?ïíÇQÉÝj?j(€1}£\?b8®Mí{?j(€1}£\?ïÔx§¨óK?`Ý"®µ¾?uì
Iʐ?`Ý"®µ¾AGN4FGL J0035.8-0837¿â;"ãæދÀQÈéᰉ À;[ø–2æÀ<´"Š‹ß@+2w÷]o?ÿ˜òtý?Óâ?»+åŒ?Їç^j?úEû7Cc@Ó³#Ñ¿ïý?üoQÇ?î|r!/¥Š¿Ý"m?ž{¿Ö3ªýD8ê¿å÷C~Ý¿ïüRáÏ=jAGNbllPMN J0035-0836?ïýêTXâ?&àB»S°?0¯.³+«"?&àB»S°?ïë9rEw?f-rA ?dƍõùÐ<?f-rA ?ïá):-oÇ?mxÌvüç?nÖş¶?mxÌvüç?ïõ°Uj7#?@9YÉf¢?TŸUœDéÇ?@9YÉf¢?ïþ¿çÈ6÷? 9Í[	Ñ?$"î%µ? 9Í[	Ñ?﯍&Í&í?øh3³?"¶Zt´–?øh3³?ïٞ[•ß?v¸9Và¤×?s0Ñýäá?v¸9Và¤×?ïÕ°)d8 ?jµ›8³?u'ë76D*?jµ›8³AGN4FGL J0035.8+6131¿ÀÖÀ…ZŒ¿ô­6À9«½¿é{À;ZÿÁße@gˆGa¾a@
{ 1ί?ÇxÐvO'?¼Š"AeÐê?ô¶Ë8x'@
(ùÿ
È?ïÿǀ²—í¿àJú¿ú+€¿è—Z$8Ä¿äöö6R¢d¿ïúú!™­¼¿ë²u"–ØÊAGNbcuLQAC 008+061?ïûrŽV´1?:²€Zx}«?B5ǯyý?:²€Zx}«?ïåEÓZÜ?v "×Ôã?jº,~«ñ?v "×Ôã?ïªó=ú·l?Ó˜_•?…C0R%?Ó˜_•?ïɇ¨!ê?`‰™âÝ?{<+Ù
?`‰™âÝ?ïûJà¨]?DmÑÐ5S?Bפ·y?DmÑÐ5S?ïA±Ë?¥âÑuAåA?—ÉÜÇ/˜¹?¥âÑuAåA?îáÞ´&}?™ä-Ý ž?¡âÒ)ã;?™ä-Ý ž?î°'hÙø?"ËN~…o?¤ýÆÞ«"?"ËN~…o	AGN4FGL J0035.9+5950¿Ÿw)Òö<ÀÖCEÏíéÀ7ñûš°À;B¬ï¡
@ $|ÍÛëy?ú•†_*2? bGÎ\š?ª¸Å-ò@
ø¤™§ÜR@'"ŽJ[?ï° F\¿Á.ÃâÃY1¿Ý­êžïÄÉ¿ÑÓ
X®ÿ¿ÛB?•—,¿Öîï!
'©AGNbll3FGL J0035.9+59491ES 0033+595?ïþ£7ìÅ*?Ô¨0†À¯?%ÌÜ¡6g?Ô¨0†À¯?ïëq"Wê?sAÏñ(þ?dŽÝ³æÖ?sAÏñ(þ?ï؟¾Ì®ð?~&¿Ûד?s° šXt?~&¿Ûד?ïüŽØ<?+ÐZFڜO?;‰:®š}£?+ÐZFڜO?ïþºßJ¹ô?!ƒö

à)?$R ™V?!ƒö

à)?ïy4•¦t?¢ôà<@M"?Ùm_¢ÿ~?¢ôà<@M"?ïÝ2}«§c?y¢ƒa¶$?qfÁ.KÖb?y¢ƒa¶$?ïü|#š—?4_g¸l,??Ì4X¾Ä?4_g¸l,AGN4FGL J0036.9+1832?ÔzBWN¬ÀFÝ/Ÿ¾À:Yºû1À<n}îBh@g*&š£@'L©%þ—?ÀCW÷ã§?¼Ìõ''5?ûz&6Ën@ªk­Î¿æÚ³ì+¿àú®/«¿æ,@Ъ¨¿çÞ¯°î¿×)9_G8N¿ïÿÁìžú,AGNbcuCRATES J003659.39+183203.7?ïÿ4ó¥?
ü/%pšX?a¡È_I?
ü/%pšX?ïòëˆ,gp?a#Cp©öˆ?Z(ïÓ, f?a#Cp©öˆ?ïôG{Œ
?TÞ²…RT¬?WÉp˜4¼æ?TÞ²…RT¬?ïÿÊÝÖ¬Â>é	‹vð'>ú'x{K>é	‹vð'?ïÿ‰0‡®?«V¥¦xä?
´†½°?«V¥¦xä?ïÄÎaU
+?†ˆýì´±"?}˜ÏuÒ4?†ˆýì´±"?ïè	²9Z?pY.àâ/??göNø%Y?pY.àâ/??ïÿ[Ð`U*?
_D'u‰?…ùîŽM?
_D'u‰AGN4FGL J0037.6+3653?ì`Ÿ"ŒŽ'À9ä—{žÀ:ÌÿؒӭÀ<t1rhÓ(@ÆXIî@$UšfH3?ÉÌS•©J?»zàÆÔ».?ðÇ#Zx›@Dt€ª_¿í¾ûˆ¡ú'¿ºÕ¢"C¿åÑÁD®[¿ØkYë-àä¿ìmˆcç0%¿ïÿÃßé47AGNfsrq4C +36.01?ïúÔEx@j?:'õW?D®éàó?:'õW?ïïÜ-µ<Z?eZ{ôZ–ã?`#ÒIF€?eZ{ôZ–ã?ïÆüÂø|m?xý%#2܍?|žŸ>©q?xý%#2܍?ïëà~íF?GPx€m/À?dê'ð±þ?GPx€m/À?ïø )£û?KNàÆöŠ‰?MYÃD÷?KNàÆöŠ‰?ïćÆ7»?'áêW*Ç?}¼r'ââ?'áêW*Ç?ï¾ÌDh?'§¬™?€LîòÆÄf?'§¬™?ïpo(y?{Lv"Y?Œ#ø5cí™?{Lv"YAGN4FGL J0037.8+1239¿¢®X½bIíÀI
¥¤i×4À9€C`§à"À<+»Ù_'G@¶I'uç@ÁªYÛ=©?­²ÿµò¿rÔåþªä?ÃÓ·79R1@z~ædùT?ïÆZAêÜ¿â咖pn¿ä›:]ôÒпà+Ôßë¸u¿ãÏß Œg'¿ã]åÄ—gAGNbll3FGL J0037.9+1239NVSS J003750+123818?ïþ´¡ö>?Ûûƒ Ðh?$µëyßìv?Ûûƒ Ðh?ïòޙJ`Ä?^s³$ˆâ?ZBÍÙ1ø?^s³$ˆâ?ïørv®ÌË?S°œ0ü?N6%Ÿ'ò?S°œ0ü?ïþè0‰k? &à,<÷?!|ú0¼8^? &à,<÷?ïþ¿ Î	?oË0"Ä/?$QŽ¶dG?oË0"Ä/?ïÊÁ˜¢^ö?€
…L(J?zŸ3š2Üü?€
…L(J?ï÷R‹#pY?^˜Þøº6«?QZê?ÏýÇ?^˜Þøº6«?ïþ~×æH? €™vÛù?(']\$Ó? €™vÛùAGN4FGL J0037.9+2612?ï6›gÏòòÀBI/Ÿ¾wÀ:×Dœè³À<ˆ')ó@+QّG@ì楻æË?Ì.sEqú?Ã'À²7J?óŒÙ|Þwð?û҃Ee¿Û@`óJ:¿à'È>Ȓ«¿ä¡wÿ•÷Ï¿è"J½¾g¿é.†%HŽå¿ðAGNbllWISE J003719.15+261312.6?ïúî՟ž?=
ŒÂ("?DGÄŒ?=
ŒÂ("?ïÖÝÔì?5¨ä©M?t'æk	[?5¨ä©M?ï°r"z©r?zärçÆPÆ?ƒãZÛ&W‡?zärçÆPÆ?ï¨ô)và¡?h–›èrR?…Âõ¢G×Ê?h–›èrR?ïè>Â)þ?eù_æ/¯?gäÁ8V¢?eù_æ/¯?ï›B2¡à?¥‰ñ'ÌB[?Œ—¹«Ãú?¥‰ñ'ÌB[?îÌao(#W?—üë™A?£9é5˜Œ?—üë™A?í`ánfÝQ? Nº¡qÂJ?´øôŒ[!ø? Nº¡qÂJAGN4FGL J0038.1+0012¿ëýò,5p®ÀO<±î$5iÀ:úûö†À<_zù›añ@»…øÒå@
¥|üªá?¶	Ê?eò?–õxί?âp¢qON@ï72œ4¿ç•¿x¿ØCûlóHb¿åCW}ÀJ2¿Óîᵒ¿âvOb=⺿â˜H+ü'AGNbll3FGL J0038.0+0012NVSS J003808+001336?ïý¥e՝?-p²Ø»Ï?7ÂÖð{¼Ì?-p²Ø»Ï?ïï9ð!ø?búYðݳ?`ïÆ? [?búYðݳ?ïë=IGØÃ?f9ªå×?d¶ö4Ê?f9ªå×?ïò«Š-…?Du• a‰?Z¨ëˆ-\?Du• a‰?ïùCsa?B8|îãpi?I¾ó¼Šr?B8|îãpi?﷍£E?‰P("ý0J?'—,_Þ?‰P("ý0J?ïê"Hvç=?p.Œ]¹ü?ek·–×2Ü?p.Œ]¹ü?ïÎæÛåÅ?i­š˜Í4ß?xŒ'†ë1?i­š˜Í4ßAGN4FGL J0038.2-2459?ÞúÔaì""ÀU–Y_í¦aÀ8ùþz¾ãÀ;ùž$BÕh@8ÃäpØZ@Q¥Ãsˆ?¦e¯¡º?¶ÎQ ï¿@aƎÅ*A@žÌíY	\¿³ÍlÚɺŸ¿Û-+|…Œœ¿äï4 #b¿âˆõý¥¿ê@N¤©¿åó4«wªAGNfsrq3FGL J0038.0-2501PKS 0035-252?ïúϺN+?GÃ!D¡¯8?G€Áñ"Ø-?GÃ!D¡¯8?ïñ_m›0j?b®'K+?]A%'‹?b®'K+?ïËóC·˜f?y¬ÕphR?z^GQH?y¬ÕphR?ïÿóïë#¿>Òzv9>Ø sKhr>Òzv9?ïú"™$?AÂâ¸Nj?G°ðt©7?AÂâ¸Nj?ï¨4Ý5Ù?‡æ¹"ý&?…òÜ]¥?‡æ¹"ý&?ï¨eùd¢?‡IǾ'êì?…恭(g‰?‡IǾ'êì?ïÿò@Ϩõ>ÛèCLÞU`>Û~Œ
Áï>ÛèCLÞU`AGN4FGL J0038.7-0204¿ç[w4àÕÀP0¬![š[À: ñ68¡1À<F"—u@Ëßèˆj@÷ÇÀ?Åd¦¹
þ?̟6çrÀg@öÇd­ÿ'@óœÚ
οËB#;"Ü¿æBM'iÒ,¿ëÍQŒºŽ¿ï݄?•AE¿ïž©£Ò؀?Áþ0\"*šAGNrdg3C 17?ïüÍÚO'—?4‹Óeiö?9',Ú#¸L?4‹Óeiö?ïâæáî>"?t²[IŒAë?m'¾ûö?t²[IŒAë?ï»Vd²ÿi?u ¤ç?*fÙoqÏ?u ¤ç?ïÛUÏr÷ø?[¸Xó;j?rU:ÕX(?[¸Xó;j?ïòñû–Ÿû?gò?[3O1?Z	@³ˆà?gò?[3O1?ï='AávÓ?¥fβ~bŸ?˜M·ÂW¤?¥fβ~bŸ?îžÝÑ`?™àÒ-ì;?¦Ní×g
?™àÒ-ì;?îR·!ê¶m?˜ò¨L¼{"?ªÔáT™4?˜ò¨L¼{"AGN4FGL J0039.0-0946?î9{"Ôk…ÀR,ºËCÀ:#ª–A…À<f=°d·:@é3þà\@u{­ˆ?½í'þŘP?¹PXÝç§?öüºÑ!Æ@û!'ÌËË?ïÿmh¹&þ¿ãšQ_™¿¿é5Ù L£¿ètSß{%:¿ïÿñ_{'?í(#ÕÈAGNfsrq3FGL J0039.1-0939TXS 0036-099?ïõèG…-Z?ŠCÖWB?T/qHì}?ŠCÖWB?ïìÙ¸~È?h…?óÆn?cp&lœÿ‰?h…?óÆn?ïÊÝ^qƒ?~\©×²ât?z'|ÂXâ"?~\©×²ât?ïï¥DÑó?NÁ/ғ?`Z»ç
Z?NÁ/ғ?ïú[ÅðÜï?J£~¹ñÈÕ?FçíîÎÅ?J£~¹ñÈÕ?ï£ó4?x?"Nõ)¹í	?‡:å1²%?"Nõ)¹í	?ïÀä¨ù—?ƒ¿ÆrùCd?¬á,q?ƒ¿ÆrùCd?g J£?B:)u?ŒfB<+#?B:)uAGN4FGL J0039.1-2219¿ã?uù×FùÀUg8}¿À:…®Ús~}À<o­é¿@ ÚÒZ*mè?ü(—ξ??½
díj| ?sUÙë9I?¶©={‹'™?ÿ–ãìÎõÇ?ïàYÜë(¿Ö8è^£¤_¿Ôb·ðœµ®¿Õ1fªY~¿ãZ7ÿuÁx¿ÅíQ½ƒAGNbcu3FGL J0039.0-2218PMN J0039-2220?ïüÊóG¤ž?*E29%ò?9¨e% #?*E29%ò?ï﫺êˆ[?b┇{|Ö?`TDøšíj?b┇{|Ö?ïòHaÔj?V™6ؼ<¯?[o<.Ÿœ³?V™6ؼ<¯?ïí̋"LJ?MådS‡ˆ?b3t¾N8?MådS‡ˆ?ï÷¶à…?I"rYþJ?P"ËÀ…†/?I"rYþJ?ï®ôYPÊ?‹çÖcZŠ"?"Bé²O\?‹çÖcZŠ"?ïó1±0—«?dù3ž<?Yœ€"?dù3ž<?ï׬í¼å?d¼·¼Qwê?t)‰žƒ£?d¼·¼QwêAGN4FGL J0039.1+4330?×*²zTô"À3M½ÙßÛÀ:¾ü‡7À<žÿ%­B@yl®)@
  ôØ?Äa1s?'½?Ú6bÂö?ýàõþõ>@	·"W`9&¿ì²ÊÃQ-?ïùZ"¡U¿á­,ˆõ¨¿Ýe¿cØ¿à/³KòG¿ïÿ8"†ZAGNbcu3FGL J0039.1+4330NVSS J003907+433015?ïý×ä$y©?3c‹¶È?1@݂óœ?3c‹¶È?ïòŸ¼O?dÅӖ
ó?ZÀˆB Z?dÅӖ
ó?ïëY0Œª?iBÑ@æÙJ?db¦¦8®?iBÑ@æÙJ?ïôáq}#u?=8¿jÓº?V=ß=v†?=8¿jÓº?ïü¿B9z9?2ô_ÿþ½?:ï'n?2ô_ÿþ½?ïˑÄ
5ž?9úÑ?z7ñÖ
=?9úÑ?ïßf¿Ÿ	=?t2OjñÅf?pL A©m¢?t2OjñÅf?ïÔk•Wô?fº¶®Ø?uÊ5l;¬?fº¶®ØAGN4FGL J0040.3+4050?Ñ*e'潩À5ü¼ßï¿@À:¸Ø£š¤À<zøØÄQÔ@!A߇O?ÿ¿ "_õ?·[±×~·¿³0M¿jRs?û-
ê¤N)@b14?èöIØÃ{¿â6M™æÆs¿èê"‡¿R¿Ö^¿à12I(h¿Å"§ŸÁ¦ÔAGNbll3FGL J0040.3+4049B3 0037+405?ïÿO =|?4¦»î\?Öö¨Å?4¦»î\?ïñ°<Úb?`¡MÎ;û?\Ÿ…ÇJÆê?`¡MÎ;û?ïúÔø³?@FƒM'tn?D¯ïbÕë=?@FƒM'tn?ïö=˜€®«?7Ъ6#ÅX?S"΀1
à?7Ъ6#ÅX?ïÿ#†ÂÒM?rñÜÎ¥?%K.ì?rñÜÎ¥?ïÏòx–?}Fú¾_::?x÷±pã?}Fú¾_::?ïøË5ünÚ?bîPJ.C(?LÓ'ýÆz?bîPJ.C(?ïĚ7½ö4?oª´a'/?}²äՙÿ?oª´a'/AGN4FGL J0040.4-2340?ĄMóäúÒÀUo@öjUÀ:˝_÷·À<š/²u2²@ÍÛLlj6@v¿yýòà?Ædô5òUH?ª"Ù…xO?ãl Åre@3¶-y
¿ºÔ뿬'ç¿èk"\Ì4¿ã³A
ŒK¿é}ÉÄڐ¿ÉÕdK3'¿ïÿס<%JAGNbll3FGL J0040.5-2339PMN J0040-2340?ïþÌ<•BÙ?¢ÅÔ?#<62à0¼?¢ÅÔ?ï玲§Ÿ?fcj1C~?`YR3?fcj1C~?ïó¼"nþÕ?Mƒ¨nŸ?X†ö¼MæJ?Mƒ¨nŸ?ïþÍ8`![?`:áE.?#,w]˜ó?`:áE.?ïý¼Kþ¹·?0¿ž2«Z?2ž°óª?0¿ž2«Z?ï¬`ø/@?ˆ ­G?"çüS";ê?ˆ ­G?ïñ°õ‰b?döꂕF#?\žïûvì?döꂕF#?ïúik\"?>c:}x}u?FZRÆqJ?>c:}x}uAGN4FGL J0040.9+3203?â+©·§>À>Ä(äû—»À;ðR
À<]J]ò$@Qmª'†W?ÿ–»cýM?ئËEäß?àEÜMsPZ@ÙÂbæ@€ðâUË?ïøIóiȿքÖ~|\È¿á¬btx¿äÏìÂ5š¿ïØl:¿å5{!ŽAGNbcuTXS 0038+319?ï÷-¡"ú×?YQQ)³ð—?Q¤¾0<áÅ?YQQ)³ð—?ïæGŠX3?i»8oo
ÿ?i¸uÜòÕ?i»8oo
ÿ?ï6/ö×|?‡_iË__B?™:1E'?‡_iË__B?ï !±^9û?gõkb]Çù?‡÷"²ÀUG?gõkb]Çù?ïð|DŽl?Z"1q!`d?_Õì©-?Z"1q!`d?ï"m\àè?'ì‰/Ýöè?Šüä¨ÇÆ?'ì‰/Ýöè?îD‹¶é?žß÷ÜKï?«¿ÇCµ‡B?žß÷ÜKï?î":Ö©?üឈDF?§¼W%Ô?üឈDFAGN4FGL J0041.3+6052¿åðÓÈrí¿ÿƒòÖKÒÀ9šN³Â9ÌÀ;Jˆ0»‰®@5T#sø@ä¬å¦¸f?ŲºÒÏEM?áúˆÇº>U@‡žYòº?öY0³Q%·¿Þ–ý]
w7¿Ë$úì.'¿èÕÃ"æ¿îÎR]ðÌ¿ämÊ=¦S¼¿ïè/>\;AGNbcuNVSS J004058+605407?éçœ(ëÈ?Ɠ÷Mÿ½:?Èa\Sèà?Ɠ÷Mÿ½:?ÄÐbýJ÷?Âñ9ôB‡?êËçz€­B?Âñ9ôB‡?çCºód?±+ á,Bc?ÐáxŠ7Î?±+ á,Bc?ƬJźΌ?ªªÍR•?êTíN'L]?ªªÍR•?ãXÉþf«?Ò>tÄ;óe?ÙNlß2«?Ò>tÄ;óe?˜Kк¢e·?¢ÏÓò£$?ï=¡yóó?¢ÏÓò£$?ß©êðEÅ?¿ºë›;|¥?à+u
‡Ý?¿ºë›;|¥?g¿ŸêyX?ZZöOp?ïè@ó)Ç?ZZöOpMIXED4FGL J0041.4+3800?Æý±Ï3ÉÀ8ÑüÁr&À;ŽK^À<©G_ɔ@ ÉfI
5
?ÿÉT!ÀD(?ÀU€ÙÚ&¿­§¤|ÕX?ï0\S½í6@½ý|(?쀏qøjà¿äŠ:N¿â֘B"пä÷bØ<l˜¿ÕœøÞbK¿Ä1ƒìÅLAGNfsrqB3 0038+377?ïþ"Êvþ†?3²Ñ#ã?'³Z¯@;Ê?3²Ñ#ã?ïó/´<vî?Z‰.õÕ
?Y —GÙU@?Z‰.õÕ
?ïóü¦{¡®?f$B­48?X²Ô'"Ž?f$B­48?ïúÀù7—?,Æ}ò¸»C?EˆûÛ\¦?,Æ}ò¸»C?ïýV@d°??3õ›äÌçÖ?5Müò®zÌ?3õ›äÌçÖ?ïÒY‰^8?X

ÖÂ?vÓ;L6?X

ÖÂ?ïù$åηš?bËŁMK?Klh 4YÍ?bËŁMK?ïâ/ª?`Îe
Á.?mïrÇþEé?`Îe
Á.AGN4FGL J0041.7-1607¿âÃÃÓmÀÀS±úëÄ	À;±¨´¿ÍÀ<ÜøÆOÛ
@!ËXàÁÌ>?ú;´4çh?ÕغEºÊ?ÇÉFZ'W‰?öIŒ\`S@DÃàj
?Ûö'¡þm?ïúeµ²¿äå\{+‰¿Çܺ–}5¿Ë­šW"¡:¿ÖÖò FAGNbcuGALEXASC J004141.24-160746.6?ïý\6??¨Ä˜Âwh?3}݃ˆ??¨Ä˜Âwh?ïíݜ¹ð¸?dóŠ ^Ö?b"cv)Ïs?dóŠ ^Ö?ïäøÍuƒ?rq›ozë½?k€(ë•?rq›ozë½?ïühUvKƒ?.þÎêu'N?<½UVŸ^½?.þÎêu'N?ïþ¦Ö÷?!Æx¹_2ê?%'+·k?!Æx¹_2ê?ï¢kÁ³ØÏ?"jׄù³ç?‡e¤7Ø4?"jׄù³ç?ïäø̞Ãi?s£h'Ô¤?k3Hg>?s£h'Ô¤?ïñ^-Nî?VÕNy~QÛ?]CÝci¥?VÕNy~QÛAGN4FGL J0041.9-4702?ïNÑ«–îÀQ­À˜$À;ã‰>ÃÀ="ÏÝù@ Ÿ³-¿Uì?úõp	}WD?Öí!zN%?ËD&J—}á?òò<ÈÞ*Ã@hÍ¿ïÿü¥¬¨¿ä¥AØèd?ïÿê›ê¬²¿Ýó"Çz¿áY®Çÿ¿Þž¼n/ÞAGNbcuRBS 0097?ïüsVl{Ý?5;Lk~ë?<eLˆVŒà?5;Lk~ë?ïôù®¤?YùÎæ}"?V¢èZAt?YùÎæ}"?ïÊ#gc;?Êâ6wÐ?zîLZÀО?Êâ6wÐ?ïúë0e"š?2'Y̦œ?DS?p—èv?2'Y̦œ?ïûº(/t?DIgb‹9?A_ ¾©i?DIgb‹9?ïÖӕ'¢v?{]К&§H?t–5²…0?{]К&§H?ï¼ÛºÈµ³?…§U&ʅz?€ÉQB/(?…§U&ʅz?ïó%)bØp?RÕPz$?Yµ¬Á\àº?RÕPz$AGN4FGL J0042.0+3640?¿gÈf5¾ÿÀ:)/ ×{|À;ò×ùP¹À<Fyaî@È)NWüÁ@ç';®+ø?ÃD&àêf¿ªñ/؊Æ?ËA˜¦ªy;?ÿ¡W¾'Ý?écànë?î¨ü
,8m¿ëŸ|!Ž›¿ÑÎû%OÅ»¿ßÍã£(
»¿á¶Í§%sAGNbll3FGL J0041.9+3639RX J0042.0+3641?ïüޯŢX?6+÷#üݾ?9
'ï?6+÷#üݾ?ïñ°}Ð#?`#€À‰7l?\Ÿ‹ÿ?`#€À‰7l?ïë*ŒVÌ&?X3$g	ñ¾?dÕs"6ZZ?X3$g	ñ¾?ïê`ùêè?KœÅ4Sš+?eŸ+j?KœÅ4Sš+?ïòÎ|4%?Wԕ²ÉZ?ZcÅ\ή?Wԕ²ÉZ?ï–٩]?"¯IæT)?~÷´©(х?"¯IæT)?ïâ´Óܶ?sš/:†å?mðK4bY{?sš/:†å?ïžQ|to¾?xŽi*·ß?ˆk âä`?xŽi*·ßAGN4FGL J0042.2+2319?æI…ýQòÀC¿rÅz%À:#ŒÍ}À<b Õb"@\*2	h@Ö×¥mã2?¾‰_d¿rF?¾Òo_DšJ?ýzŽ ¿"(@ø­ˆÛ0¿Ÿ»Þ#G"ú¿æ²g'Ñ`¿ã$e¥vF®¿äšŽ:!¿è@*'_–>¿ïߏ@zAGNfsrq3FGL J0042.0+2318PKS 0039+230?ïüIÉïð
?:ŸùVã¯L?=±®ú,?:ŸùVã¯L?ïð'O¥.Î?^G¹._»ß?_±`&Ãø?^G¹._»ß?ïë©t0\?j'£ÃA?dV‹åt:?j'£ÃA?ïÕz¡9~¯?Y"Xˆgx ?uB¯€ÍL$?Y"Xˆgx ?ïmìYÚçÃ?—ÖÑÁg;?'Bt½Ã϶?—ÖÑÁg;?ï¾/Ðþ	Ü?…œs
ô?€t̄+?…œs
ô?ïœ9çŠò?Žš¥×AO>?ˆûñ—KOx?Žš¥×AO>?ïATü†£É?€ÄÊ~9Ô?—Õ`wŒá?€ÄÊ~9ÔAGN4FGL J0043.5-0442¿§´]ŠÅÀPߊ\å´$À:æ~Ä+=›À<†,:ñn@ š:ë
š?þ Aׁ\?ÆÐ\cÙ`?¤âcâÓt\?á­»úíqˆ@""xB[ð¿ê?.8¿âÑBþ,kC¿ã'·iŽ9¿Ö
×YÉ¿àý­_Ÿ!ï¿ÍïªGfÆÞAGNbll3FGL J0043.5-04441RXS J004333.7-044257?ïþびãŒ?¯
#&Ü?!Çåð9?¯
#&Ü?ïîÊÎùUu?i/sñvrÌ?a51"'kV?i/sñvrÌ?ïöäá¯?>‹¨²½É?R7ÖB°Áa?>‹¨²½É?ïûk=21ù?,òæÏý•Š?BS
@$?,òæÏý•Š?ïþÍ°U?Šw'^?#$üL,!Á?Šw'^?ナñ¾k-?ƒŽ=Ð-?€^ƒ€—ð?ƒŽ=Ð-?ïû?Õ
¼z?HÉô¥—?C«>#?HÉô¥—?ïé‰Ë½¥Š?ZGIòe®H?fv4gv=í?ZGIòe®HAGN4FGL J0043.6+2223?ØEFÌÿ2âÀD9‡çÀnÀ;¡"úÖËÀ<'g†!Ñ@†Ã>@=–é»ðÜ?Ò£9UŒ$?·iþ Õ®?é=[?Á¶ï@¾†ù¿ïØ ó•Žr?ïџD~_¿à¢wžÈ·¿ß.8øo¿áéBžá7¿ïþΈ°=AGNbcuTXS 0040+221?ïþԚ²¯{?PÏõ)ο?"¶U™¢ž?PÏõ)ο?ïñ68ÀÞ?]óÒê¯÷?]"ÿ8ó"?]óÒê¯÷?ïóS6*V?JÈ|!rÚ?YÛYYñä?JÈ|!rÚ?ï÷l—œ®?6HƒFËI»?Q&Тçðm?6HƒFËI»?ïÿ6ö{
Ò?ÝÚÐ֐?!+æt?ÝÚÐ֐?ïÃÉ_ý8?…oYÚ/ïƒ?~P´?…oYÚ/ïƒ?ïì´xÓ?iÅíëˆf?cKˆ kÌ?iÅíëˆf?ïÞ6Ž~ÕÀ?bãÀ%iÜì?pä¸ÃTÏÍ?bãÀ%iÜìAGN4FGL J0043.7-1116¿ïD"†YmQÀRƒ7u¸À:șI—#À<ˆÊ½ÿ@ )Ð3Á?ùz@Ù#¯?Óì'?
?Ñ"‰âíJœ@¢Pr[@}¢×/ý?ïÿŸ¸fä¿ëa¯ÐâÜ¿Ù5 uÖÇ¿Êò*Z~&¿æØåÿùŸê¿ã‰!Q^lAGNbll3FGL J0043.7-11171RXS J004349.3-111612?ïþN‹I? Õ§Üñ'?+ªDKÔv? Õ§Üñ'?ïíކÍRó?eÀO"ƒM?b!xÿÒÔë?eÀO"ƒM?ïâWËÃãD?pw~B?m¨4!ÿ³ò?pw~B?ïñ<G¦T5?D=/ÿ
?]‡pi c?D=/ÿ
?ïþõ¦,F|?å£öNWO? ¥œìîó?å£öNWO?ïÀ ßýÝ?ƒ8"áŒ?ïúœYa?ƒ8"áŒ?ïåù›¯?ë?s…‡(Qҋ?jdøä3?s…‡(Qҋ?ïÛB¦\?b‡~™K±?rtޕt`m?b‡~™K±AGN4FGL J0043.8+3425¿Ê¹IÂì¤.À<j|¦CÌÀ8b–›¸XÀ;'U¤wC-@^[/¦Œ?ýÓèPïÝ?¡kÉýQ?ªs‹_fN@
¾•ßе@ýýÃå~?ïÿG©ýd¿Ø\4ß/ÐÓ¿àíØJ¯P»¿Ù·ã܈׀¿âÝÞQ"'¿à°éAw™•AGNfsrq3FGL J0043.8+3425GB6 J0043+3426?ïþÆ)Dœè?JÚõԊá?#g³?ß?JÚõԊá?ïñç­ë®?ex¢+ûÑ?\1𿥄Ð?ex¢+ûÑ?ïå˦²÷?n%öi)È?j4Yx•0µ?n%öi)È?ïý¬¾rN? ñŽ× Ál?2šö&A? ñŽ× Ál?ïþý‡»ÜÌ?R'DÙ^? 'ƒ¼R?R'DÙ^?ïÍP•¢G?~:aÅ«¼û?yWÀ݈?~:aÅ«¼û?ïäìZJ"?w2¶¤U?k¥ð†7­?w2¶¤U?ïü˜#ºM?0=¼¼"Î?;?`?0=¼¼"ÎAGN4FGL J0044.2-8424?™q=—ÖšÀ@\¤~Ïé¸À:P"Þ™À<:Dfa]é@Ä9Ö:Š@JCþ\'Ñ?À4	òÈ	?1SW''»?ÐU@0ÞP^¿ßB™¢ÓÔÿ¿á€Ì¥Wh¿èˆ^Þ²¨¿ëÙY_ç¿ÇbT]û2ç¿ïÿ`}™2ìAGNfsrq3FGL J0046.7-8419PKS 0044-84?ïþÞeâ™#?»'ViÉ?"¡aáv2?»'ViÉ?ï÷&`£(?V-"y€‡Â?Q³>›› ]?V-"y€‡Â?ïæï36€?pmò¾MT?iÌQŒð€?pmò¾MT?ïÿÛ¿¦@>áÈJ'Ù>ò JÛo>k>áÈJ'Ù?ïþ9Êã#â?0‡QöX¥?,cOØaB6?0‡QöX¥?ïáàê)î«?p4ÇϹD?ni¬ñ?p4ÇϹD?ïÍO,ý¨Ò?b¸.c?yXiq]cQ?b¸.c?ïÿP	؛ã?ÉlŸ¿­^?þÅcBíˆ?ÉlŸ¿­^AGN4FGL J0044.8+6802¿ïR{Lý^»@²{²þÅmÀ9ÈÇÜ$YÀ;¡óÒvZ@ו#SÀ@N
Ää ÿ?¿TWñ?³S¡èÅ?õÙ	†'@éšòŠ «¿ÕßGŽ4
Ê¿ŽXkã=í¿éùù î?¿áx7Ÿ(¤º¿æPqgKh´¿èë»MlšAGNbcuLQAC 011+068?ïü˜5&¹Ž?36%Zr\R?;>VƒÕ&½?36%Zr\R?ïç
°Ý%?lbÀQ"Ñ?hõãb`«e?lbÀQ"Ñ?ïٌƒ†‡Ä?t´=±QÌ?s9¾TuÝ?t´=±QÌ?ïÙyVê-Â?S!,顨Š?sCT…i¿?S!,顨Š?ïÒ':_*?€LΚÄEL?vìbá™?€LΚÄEL?ï,8Â2N?¢s@—n?šx纒LC?¢s@—n?ïC«!<¡Ø?"‹.ûH¾¾?—Š›ÓD[?"‹.ûH¾¾?îæuül³Ä?ŠþmÙ¢H??¡˜ 6¡É?ŠþmÙ¢H?AGN4FGL J0045.1-3706¿ãQ>܉®?ÀSûί%À9µ@+i:VÀ<†ãlK'µ@çoÚX|@¡–EQBé?®©é…Y?™€öà^?çœAƆ@†¥ªõ·¿ÏȆŽàÙ¿æ4B'KÇ¿çÖø4Y£à¿èå—ží–¿ì '¢ s¿£.üÓТAGNfsrq3FGL J0045.2-3704PKS 0042-373?ïþ–­ùDq?3™ß"Ay?&•›ºxš?3™ß"Ay?ï÷qÎÏ[r?V¨¸†æ*?QbçùÊl?V¨¸†æ*?ïæ#rËÏw?k¥±åF¿?i܍NM'?k¥±åF¿?ïÿƵ«G>òÿªøð>ü¥wâ6>òÿªøð?ïÿ&¿î~4?ȯì̃?(œYoP?ȯì̃?ïÜ¥*¤ø?s¤ÇÃÎ?qò-w¼?s¤ÇÃÎ?ïä+p®ü?sòSȾ×?kԏê'Ta?sòSȾ×?ïÿ}Ø.;
?
âM¥´º?Dô´Ø€ñ?
âM¥´ºAGN4FGL J0045.3+2128¿¸^FàÙKÀD°üó0À8Ýi¸*~YÀ;œñ-Õ%a@¤zŽ¤h?ú´‡Ç	>m?¬º¢}ÃÐ$?³ˆ¹ø^Ëè@ZÂß
A1@žA|Í,?¹Jˆ ‰3+¿Ø/õ;*ùS¿Ùåpݍº=¿Ño¤}£Cç¿â9ʑ‰)à¿ÕT•cT
HAGNbll3FGL J0045.3+2126GB6 J0045+2127?ïþØÌp—©?DO2'¯?"s<¬Òó?DO2'¯?ïòúŠŽþz?]™Ð†•ë?Z
ëOö‹®?]™Ð†•ë?ïï¯ì¨pˆ?YÐ\9õ›?`Ph
—°?YÐ\9õ›?ïÿr"KO>þŠØ?éIa?»³©1+B>þŠØ?éIa?ïþðr2;U?ÙÆ>þ°? øÞ®|9?ÙÆ>þ°?ïÇ\ã…ËÜ?…¨"¦üŒ6?|QŽHȽ¿?…¨"¦üŒ6?ïíÌuM	?löBTtߙ?b3‹‹ï(?löBTtߙ?ïÿG t÷p?>Âz £'?î–ÓÔÍ?>Âz £'AGN4FGL J0045.7+1217?˅îC6'ëÀIGD#‰À9QË(‡Þ†À<IbI¡4@¼ÇÞ{uí?ÿPUhaQ?¯<òN¼{œ?•(%Ž.?çs÷+E(@ÿz'î.Ç¿ØPQÜÁŒ}¿âI¾ó(¿Þ¯îºÞ7Ù¿à')ÜÓ¿×âš~ñ͍¿ä[³"ý*cAGNbll3FGL J0045.7+1217GB6 J0045+1217?ïþÛN$N?0Ù¤H1#?"KW"¶ñ?0Ù¤H1#?ïó½ë™§Ã?WôŠH?X"(±3›?WôŠH?ï÷äeI?boÊHí%?QÀ7KDn¾?boÊHí%?ïþkg?ê†öÈ?)I‹˜ÔÍ?ê†öÈ?ïþAÿ[¯? øwrTD?+ï3"ßɺ? øwrTD?ïÒ/Ï?\¦?€a&À
?vèuŸ@Ü?€a&À
?ïøK÷Wî\?\ð¼'Ú?NÐ#žCGÈ?\ð¼'Ú?ïýB¨ñü1?+ªê¨¬?5êº:†Ä?+ªê¨¬AGN4FGL J0047.0+5657¿ïb…ÔêžÀ 2@Äì.À9'RYi'âÀ;áJóCY@Äé÷U @"úC'œý?³õõ d4Ä?½ü`‰ê
@	,žÄ{Å@ý¢Žø×?Ôy™ž÷ýR¿ÔúŒ"¸'¿á»´v"±Ó¿Þ­' ­ßø¿å`s^™¿è fèlAGNbll3FGL J0047.0+5658GB6 J0047+5657?ïý…Aõ]?0\Fȳ4Â?3×Wš–?0\Fȳ4Â?ïÅÔ?jF"'#PÙ?acy<N[?jF"'#PÙ?ïí_"e'L?d®\e,?b kÚƒ‰?d®\e,?ïúžûC?*âÿV¯ò+?E"2N?*âÿV¯ò+?ïûËÁE@??ÙRÊå?AÈЕ6??ÙRÊå?ï®bО'P?ÆÌÛúâì?"gKߖ™Û?ÆÌÛúâì?ïצ"?|™öø£¡ý?t,û¢T~‰?|™öø£¡ý?ïðLnÌ&?Jâ­Š°?_g"+T"¿?Jâ­Š°AGN4FGL J0047.1-6203¿ãyIbÓ"ÀKˆÎp:ûÀ;3&yÀ<‰ÿæՌ@S1j0Jv@	]"à¤ñ?هö#]RA?äiTpš?ú¡#K^£$@k%mL߂?嗀Œî;¿êŒºùe²¿ïü£õ=._?íSÀì÷¿ïZ¿Ï
o¿íã°> ÍAGNbcuPKS 0045-623?ïÂ!Kí
?"ƒŸ)?~ïZœÕÍu?"ƒŸ)?ï–ŦŠ:M?˜á '0»B?ŠN–]ql¡?˜á '0»B?îÀ=¿ Œ?œ\ˆÔëÎF?¯³ü%½ÅA?œ\ˆÔëÎF?﫝%ø'?~0é
ŽÝ?…¶®s™?~0é
ŽÝ?œ‰|Û?ŸAŒ<cÞ?ŠÓ˜ë_9??ŸAŒ<cÞ?îY_¨î2?¼˜ôÌ"á_?®êjÝgë?¼˜ôÌ"á_?팾Ë
ž?¢»«õä3¡?³š	¥Š?¢»«õä3¡?ê}1+úX?Â_Èûº?Æ;PÊ ?Â_ÈûºAGN4FGL J0047.9+3947¿îL~Lƒ‰À7¶o"5ÒÀ9uÓú¾wŸÀ<*¯ZËþq@¬Ë"œ?ÿ1è_ÐJ0?­óÆB"?œi³Å6Læ?ðw_²íþ@»4‰tˆh¿Ñ	£¢†þ¿áHÅ †l¿ß®¬:Ûô¿ßj
 AÿT¿Ûä:|¨¿áª	µólAGNbll3FGL J0048.0+3950B3 0045+395?ïÿ=û§ð?]îjÌ?Dd+‡Ú?]îjÌ?ïö¹°}?V`•¾9À?SЌnf¦¯?V`•¾9À?ïùˆà—b?@'‰€Å?IÜ|þ<ƒ?@'‰€Å?ïþ©ZEµ†?â¾Ïâ¿?%j^ÅnS?â¾Ïâ¿?ïþ׋d'?ORJ/?"‡Mà("‡?ORJ/?ïÔPݛ¯§?|Bk>x?uב<wr?|Bk>x?ïù"ùy~?Zó²(Šv?Iì;í¡?Zó²(Šv?ïýË)V?##-;:
ö?1¦¶{òˆ?##-;:
öAGN4FGL J0047.9+5448¿ïزކ€À "q›MÏÀ;MHœQÿÀ<¥;Ϲç@#—/£†­Y?ùJ?Ú
¢ñ?Å …œº¿tˆÏ-5~?º´÷ Þ@íšü?ç–º$Sœ?ïþ¡ÆŽÅ*¿êZ^gŠS?âúÎÓ7J¿Ý=–ä]$¿ÆÑ>¶ôô3AGNbcu3FGL J0047.9+54471RXS J004754.5+544758?ïþµbøÉ?%êlW8è?.T©vJ'¸?%êlW8è?ïó:Oº°ô?\ë1z?Y‹aNÇ7?\ë1z?ïßÅ""w?u¿XN¯hH?pnÚºx?u¿XN¯hH?ï÷¼ö±Ÿ?@œ?´Ú6?P†tåÑÊ?@œ?´Ú6?ïúòƒ¯fN?CGB저n?D5ð±ÐÑ?CGB저n?ﺟ>°P&?*Â^#?X0]2è?*Â^#?ïÎÁ¯•âÞ?¯›œÿ®º?xŸ(& 4â?¯›œÿ®º?ïç[ÐKÝ?c~U¢÷Ü?h¤êK1Œ?c~U¢÷ÜAGN4FGL J0047.9+2233¿éËÅXHÀD&™Øƒº4À9àGÐy)¸À;é•é
ðõ@H	 <Ëã@åäËÇ?··Rèa?Žá‡Ÿ¤©?ØÇW­eÿ8@UC#Á%O?ç(å!,u¿å˜|··ð¿è¯;Œž"¿â13~²†¿äñˆ£¨U¿ïþÛÝáÈAGNfsrq3FGL J0048.0+2236GB6 J0048+2234?ïþ™úx½½?ÚЧ­©Y?&`YÞyá?ÚЧ­©Y?ïôÂSïbÆ?WìOԌ³?V{Xy0s?WìOԌ³?ïòÑ´ài?X­Ÿ5Á¬?[Ê\¿z}?X­Ÿ5Á¬?ïÿ¥G€OÏ>ö;ø¼àÊÅ?®'ÅIŸ>ö;ø¼àÊÅ?ïÿ=qòØò?Ñ*_W?Qȋ"°?Ñ*_W?ïÏ­‰²é?{Ï܆‡"Þ?x);@¨{²?{Ï܆‡"Þ?ïæ^>cq?p¸(lÝR?i¡éÉ۟Y?p¸(lÝR?ïÿC9*
?‰½A:Al?˜âd‡–{?‰½A:AlAGN4FGL J0048.6-2427¿ï+҄zV;ÀUÐQ£"îÀ:×{‰äðÀ<¦WF7ò¶@Dú¦#ë˜?ÿ¡¸·lx?Ä~´%Œª?º5‡Ì<¯?õ®žä\6@VÇâØ'?ë1` (Õ¿ß[dc¿àgN"¢Â7¿á÷7…¨K¿á¥ø¸
"'¿à_`îWaAGNbcu1RXS J004836.9-242631?ïþŒé:ŸA?õüW?'1iڇiD?õüW?ïîÙÞÇåÌ?d}`J¼ë?a&!{r‹'?d}`J¼ë?ï÷ã"|Úz?BÕ&kã?P8öËx#@?BÕ&kã?ïôTuÎ
j?<Åq—E?WW!ì­?<Åq—E?ïþEÂEÏ?"¦9üC­?+£Ø‡¾-?"¦9üC­?ï²ÜÏàc¿?Š»"óË?ƒHÌåÐG?Š»"óË?ïó±́?jó'úQ?XØ.C?jó'úQ?ïÔè!…­?bÝðݍ?u‹ï_]­?bÝðݍAGN4FGL J0049.0+2252¿î^Þ`?}ÀCÿU›=ÈÀ:Ýeõ'^êÀ<<À%z@éíÞjY@œ©ïR2Ó?Ê ½šTÕ?¥‹"òe¸—?ÞVq[Œî?ÿ[ˆdpm¿î`ýÀµ'?ÕéxÔýó¶¿é#"¿lçà¿âü	Ñ:׿Øã_5o£¿æ}ÆUˏAGNbllCRATES J004901.37+225315.4?ïýÄ·ˆ§?)"gùE÷?1ÚD³7Ê?)"gùE÷?ïíÂÛÝ5ü?gÙOAÿ¥L?b=$BflE?gÙOAÿ¥L?ïë³:ï.?dï
o³¬Á?dñLÆp©ï?dï
o³¬Á?ïóxCøA4?A¨8±® Ð?Yxaô8b?A¨8±® Ð?ïøGeÍÃ?U,G¨ZZ?OòâÀ¾ô_?U,G¨ZZ?ï¼[΢?…Ž"å÷b?€é9™¥~?…Ž"å÷b?ïáIœ‰Á"?wQزژr?n¶cR'}L?wQزژr?Òrq?}õ¡V?ŠK‡r7›?}õ¡VAGN4FGL J0049.1+4223¿ïö¼5¥ÔÀ4zÅ;ËÀ;*|næg©À<³ÿþR€Ö@ ×âæê…D?üQ¸> NÀ?Ó Iaûc?¿ ãdéº?ï-Ú-Þ_œ@|Eœw?ï¯2Ú˓¿äut¡<¦$¿è$cÂG7Í?"UM[ÊÎg¿á¿m~2µà¿á6ߐðAGNbll3FGL J0049.0+4224GALEXASC J004859.14+422351.4?ïÿWwqaÓ?lÛûØÆ?4(
w?lÛûØÆ?ïõŸi3Ã?]6y¶ê«7?UøÀÅ$[X?]6y¶ê«7?ïøÚð
U?Sl¹böé?L—¬€©²?Sl¹böé?ïùé%î?.,ŒY'Kk?H[kûҐ?.,ŒY'Kk?ïÿ§V+ìÔ?«¤ ^¡†?*f…¸¤¾?«¤ ^¡†?ïÓ¾Ðؤ?zæ=æšE?v —s¨Z?zæ=æšE?ï÷疍ܳ?cÒst%Ê ?P0Ó*ë^?cÒst%Ê ?ïì8í~Àr?TøÒ`àç?cÇiâ6^?TøÒ`àçAGN4FGL J0049.4-5402¿Ù÷47r»'ÀO‹e<š»À:v©ò­1À<®Ð"¢§@Nu*¤n_@j<÷T?Á¨òÒðÓ<?Â.À‡ÅÙ?ý­X"?…@n>§Z¢c¿å3êH֎¿Ü–AöD•[¿áM¦ a4¿áVÊýiͤ¿ã±—¢H"Ä¿ïÿæ4|ßOAGNbcu3FGL J0049.4-5401PMN J0049-5402?ïûˆ
"È=?6Æ|Ë]"?AßÖ0CLþ?6Æ|Ë]"?ïô6H;ƒ?ZOßßù£8?W"oÿ,sŽ?ZOßßù£8?ïèæÖ¹4¿?fnåTÛD?g)rÆ@I?fnåTÛD?ïòâ¸=ëë?Auªÿôa?Z:&²Éý?Auªÿôa?ïîèM†Æƒ?[s'"»¨Æ?a²¸rLw?[s'"»¨Æ?ïΕj9I?ƒyÐæ¶Ó?xµukߛŠ?ƒyÐæ¶Ó?ïÌ=*‹w?}d͜²x?yÀaj
XF?}d͜²x?ïÀ.qŸè?phømã¨ô?èǏ®+Ê?phømã¨ôAGN4FGL J0049.5-4150¿ìؓ¯ACÀRÑÀÁü2À;pÝF—"À<ÛÓÜí@ [k¤hՁ?þìZ{v™?ΒÉ[S7à?¬RÚ?âeIÀé>È?öÿ¶ßO±C¿ïýà5_]^?ﶴÝlØ¿ãN$ É8Ä¿áÅGMƒA¿Âh±Å4}
¿æ%µÁÃY\AGNbcu3FGL J0049.4-4149SUMSS J004938-415140?ïú-hÌzË?zfŒí´Üë?GJ]Eí™À?zfŒí´Üë?ïðŸ9ìŠØ?g5'bVî?^ÁŒŒž¿?g5'bVî?ïê}¯®.?`1 …òÍÜ?eå';´*!?`1 …òÍÜ?ïùÁãöÆ,?8¤CpC£Ä?Høo,)?8¤CpC£Ä?ïþ7ËÉA¨?15Ð,Ý?,ƒDÀ¾¿u?15Ð,Ý?ïŸÞ"W?š=Ö"¬•Y?ˆ<i¼úJ?š=Ö"¬•Y?ïá|.=À?uIwZ
"?nƒÑ¿¦w¼?uIwZ
"?ïÕk¯?púÕ¡Å%¦?uJ~D¦½Œ?púÕ¡Å%¦AGN4FGL J0049.6-4500¿æ'ÆnŽÓîÀRo~=ÁÀ:ØúÕS"À<©"3(Ky@NÇÉ-@©WÚ²h?ÇlJ«õ½?®»¬¾åXŠ?㟮†¨Y@Óz›§Ó¿±V
þ'¿æ̬€üꢿç{é»â¿çk|·¸¿ïÿÿ" 5•?èiÇy¦µAGNfsrq3FGL J0050.0-4458PMN J0049-4457?ïúÒUf¨š?K˜(¦¬?D¶ª3cÞ?K˜(¦¬?ïòM¬[=?f¼«ðq?[ïdœJŔ?f¼«ðq?ï¨Zý|˜?‡òÅ]Vm?…é@«(Ó­?‡òÅ]Vm?ïù1,ép?;"µÖsç?K;NˆÞ(¸?;"µÖsç?ïøÁOk"8?W=j˜µ¦?LúÂ24?W=j˜µ¦?ïº]þ|¶ú?'¸9SÝ?h€bŠ˜?'¸9SÝ?ï°Ü.)û?…)ÔÈkT'?ƒÈôSŽf?…)ÔÈkT'?ï¼$$'H¬?uõQ÷Q¯B?€ööÑ?uõQ÷Q¯BAGN4FGL J0049.7+0237¿ìöÙЍÃðÀNï
å6PÀ8íeéŠsÀ<	"¾pé@° í@P'½´+?¦\‹œ*îk?­ODœù0¿@CjÆGwŽ@þÓºÒ¤R?á' ù	kº¿á'[åY¿ã›.Y¯ž¿¿ák7†
¢¿è'Ì®š¿åÀ×@n/3AGNbll3FGL J0049.7+0237PKS 0047+023?ïýüJâ…?('ݨWƒ?0-åd÷è?('ݨWƒ?ïòFˆòÐ?]p
Àð?ZýsNOp
?]p
Àð?ïæ6°–5a?tb·ö ?iÉOŸd†«?tb·ö ?ïüÅ´Ò?,†­|®é?9ÒYÉT%t?,†­|®é?ïü™Å¾Ã?2ò|Ù7Ú?;1ØÛ!ÐÇ?2ò|Ù7Ú?ïÆI×Ô+«?ˆxb`5?|Û1g
Ž?ˆxb`5?ﵖw¦)Ë?"HÞJ‹"ý?'šb5=G?"HÞJ‹"ý?ïúUáø?B	Äa
?G²§«›4J?B	Äa
AGN4FGL J0050.0-5736¿À3eÞPÞÀMÁe^(ªCÀ9¾®"½š*À<gKrÅz@k"K÷¥@äwC-|:?°ZöƛZd?f7þ…<Ñ?ÎVüfŒ@¿ü'Çðð¿ÎÑèÀsM*¿å!aña­¿éÅ%nO¿åÀ–'õ¿æQtœŠâ¿ïÿ¢AÞÇ¡AGNfsrq3FGL J0049.8-5737PKS 0047-579?ïþ®µú<5?Ùv–$å–?%ŸjX)]?Ùv–$å–?ïø‡
ÿ@?Nj_¥T»è?MãÓñôº£?Nj_¥T»è?ïæ;í°¶Û?t¼øOrŒ?iÄ*-\Ñ?t¼øOrŒ?ïÿ¬¨6?'ºF 5?ËwÚ7?'ºF 5?ïþª«m_2?%Þ=·Æ?%UDð!…±?%Þ=·Æ?ïÛK;xã'?€›_¬_ÝG?rZbEž0‰?€›_¬_ÝG?ïÝA.üö>?z4ñú-Ù?q_hãxû?z4ñú-Ù?ïþä2UMö?ÈvZòž?!¼Û³—þ?ÈvZòžAGN4FGL J0050.4-0452¿ïÞøڂÿÀPð¼£À9 ܝ$h•À<cæYeÍ@"Eò¨@¯ÁÄ[D?«¿ gå©?±·ðq@­¶åû7@R҄ǥq¿Ïá
?x¿âýW^‹¦'¿æOµë÷ö¿áï åRÖ¿ì—tË"¾¿ä¡Z=c7ÞAGNfsrq3FGL J0050.4-0449PKS 0047-051?ïý…"H¶?$2ç–:¤?3ӕ¯ë¶"?$2ç–:¤?ïñg'Л?aÃôMҖD?]0Ú_i¿?aÃôMҖD?ïޟ!?ö?x'ø ?p°o(Á½?x'ø ?ïÿ$æiV?
–ó±r{?c0¢L1ð?
–ó±r{?ïýÛ¿ü&N?%
QWê?1!ÿ¶Yoê?%
QWê?ïÊ5N§"?ƒ7r«Ï¡?zåXÄC9±?ƒ7r«Ï¡?ïàFŸ Â?t+ÇÉu±à?o¹`՟¦?t+ÇÉu±à?ïþ&™ûFæ?%	)ƒÀžÞ?-–dz~;Ø?%	)ƒÀžÞAGN4FGL J0050.7-0929¿ïlÝúØ´ôÀRSÞ¤e¥À8Q'M›À;\ΌÀmC@Q(ÜC?þ¼~ ïÏ0?œ‰8DâT–?¯Ið !Ú,@§¾öJu@?¤T¿?"Ç9¬L­¿×£I›ªjø¿àø%
{"¿ßÛ¿PãG¿âiTWp)^¿åP}'%VÒAGNBLL3FGL J0050.6-0929PKS 0048-09?ïüïÎÉ@?4/Žùum?8‹Wü—?4/Žùum?ïìÓö6Ó?gžÛ®Ú!?cã,	É,"?gžÛ®Ú!?ïçö%P?lF
T-…õ?hìê#÷¸R?lF
T-…õ?ïû^ZÓ|?. ~"Øœ?B†—~??. ~"Øœ?ïýó3Ï÷`?("(Á¾?0fa-Îa¦?("(Á¾?ï¶{‡éK'?Êøh/_?'aý/¶?Êøh/_?ï牃™IŠ?xW92]è?hv|w4•å?xW92]è?ïò¯Šû#Ö?LVGÄ¢Í?Z é¦Ã"è?LVGÄ¢ÍAGN4FGL J0051.1-0648¿ïm†½b»PÀQk˜ñÓíRÀ9r}7%À<©&¤¯@€|ªEä@ÜIwBV½?±üàeÛÑø?ÃïÙÂ(¯@ÔçhY…­@Sš±ÇŽ?ïøÇǪN¿á½KÙÅÚ¿ä>Ðñ¼¿ç]žk»¿åv"@Áç¿ïún×S9AGNfsrq3FGL J0051.0-0649PKS 0048-071?ïüjb§ô?9ýµH??<®à úÑ?9ýµH?ïð¬åô?b_#àZ¢Q?_ÿÀ0ˆ•?b_#àZ¢Q?ïÓÑ7âç¹?q·Vœ•"?vcî?ÏÖ?q·Vœ•"?ïüjFS²?'€bCh~?<­Ïð‡¤?'€bCh~?ïûA'¥P?A=$zDÞÄ?Bù´sÊ&F?A=$zDÞÄ?ïÂ$Q»Uù?ƒ"¡Ν_?~í×9²[6?ƒ"¡Ν_?ïwä¾3Ç?Žl©þ?^?'h6<?Žl©þ?^?ïôv<(á?Hªº7g{?WÛê¢ü¿?Hªº7g{AGN4FGL J0051.2-6242?ÉïfˆRÒéÀK6W}•WÀ8¨ìëPE"À;š‡–ü@ÉI®áÂ?ùWêï̓?§ߜ]?¸'\»Aßô@¢:lãX*@hη	?ï1Çù(uj?Ðó=å=ÜÚ¿ÔæФGÈl¿Ók={5«^¿ÛýÕî´~!¿Ý̩܇ÕÍAGNbll3FGL J0051.2-62411RXS J005117.7-624154?ïû#6]V•?B}@ðëëZ?Cs&9H‡P?B}@ðëëZ?ïô[ÉQ?`E`lßIÐ?WHnSNÂj?`E`lßIÐ?o©º?Œ.ðñSÆ¥?Š'ÿ6YŸ?Œ.ðñSÆ¥?ïý4¢ZCª?$þ,ëÄRa?6Zíõÿ%Ô?$þ,ëÄRa?ïý¬¹1–?-®	™gœb?2š5`D¬ö?-®	™gœb?ïÚe¹d²?w9p£Nù¶?rÍ#`䐞?w9p£Nù¶?ï½FȼG?Šn—¡í‡?€¹îR b>?Šn—¡í‡?ïú}B(¢?9«7™°j?F
ö†ƒWP?9«7™°jAGN4FGL J0051.5-4220?Ò'55c['ÀR²~|âÀ:Ju†"ÚÀ<vÀ5¯å@3"±¨Y%@rhż7S?ÂítAVâ?Ñô>Á0âK@	æb I@	sM힩y?çÃßoŠ¿å­çχ'0¿êRª\_|g¿îô±ë±¿ï5ç­ù¢ï¿íO›ÿO€òAGNfsrqPKS 0048-427?ïõº#ÒÃ?xbtÙa«Ð?T‹¸6¾>?xbtÙa«Ð?ïéœWJOì?oM'LKǤ?fc¨Ë­"V?oM'LKǤ?ïXø
\"Ú?0QÆ5Ü?"àþY£¬?0QÆ5Ü?ïáÕ<Tf?X᷺ͮ÷?n*ÃÍõ–Å?X᷺ͮ÷?ïêHCÍ?kˆ¶@C?eøô‹Á3x?kˆ¶@C?ïb#"7c?›cj'¤§?Œ'w(°—E?›cj'¤§?î«~C´é?œ>áœ?¥HÌ ˜l?œ>áœ?ïMqÓ&?ŒvœýAØ¿?–Qؾ1N?ŒvœýAØ¿AGN4FGL J0052.9-6644?Ý)4Á¤÷ÀI28ÅCÀ;DʈNî{À<ô±v/@žë‹©ÁÛ@m‹Ù½v?ĹÚVÎû¿RqÔ®˜"?‹,1"Å«@d3¹jð¿ã_mži3¿Ù(À]ӚǿæøÀ$óª¿ÎïA–Î82¿â ³Ô®Bž¿ÛÖò FAGNbcuPMN J0052-6641?ïþýò? ™îOâå5?.%ß¡‡m? ™îOâå5?ïö-a³é?T¥üu$M÷?S¥ÁP]Í?T¥üu$M÷?ïóè'Iè?TCZšêÍ?X/=ùP?TCZšêÍ?ïý³?ï‡?õBŠ?2fÄ–å?õBŠ?ïþ2E!4?!¸Š§ÜÉ*?,Û±­¾¿ñ?!¸Š§ÜÉ*?ïÞ€¹	2?q:³ÅÀÅ'?pü?—Ï2?q:³ÅÀÅ'?ïø*ì#?XõÇð'~?M¿TšÄË?XõÇð'~?ïõsë<Ø?F©©µ-7]?U)b"½?F©©µ-7]AGN4FGL J0054.4+8627¿ì«b%Rä˜@7"æŸê%À:ŒAÂB/À<zxQJ@Gœ£º.å@Vº «q?Âàßÿ.žÏ?¾Þ"4³;?ô׿T>E¶@'õf?íâc¢fǵ¿äê>xâ¿ç]?`¾à¿ìiD#‰¿ïÿýaw?ïÿéÅ+ÜAGNbcuWN B0046.2+8611?ïûœ.'?DŽÕî?AûjÓ?DŽÕî?ïðY.'m?`ü8?_Mǝ[Å¡?`ü8?ïß¼çãÃ?jl95Âí?p!‹ók*œ?jl95Âí?ïиt?b™ÓX0³q?wóóIh?b™ÓX0³q?ïéòÍðí?j"¯-UQÚ?fæ
^
þ?j"¯-UQÚ?ï§z:–÷?IÓœ?†!zÿ²%?IÓœ?磻ťCÏ?†øeÈTï¦?†–Κ¨ ?†øeÈTï¦?îj6/?˜$Ͻùèg?©\Êí1?˜$ϽùègAGN4FGL J0054.7-2455¿ê#óPÞلÀU놘5ŒÀ9igH
¶À;õ8Lw§×@ %"O…y?úîuÿ`Ð?±YéA¢?³¨Ö£eJ]@-J¡!@§
fÅÜÄ¿æi'z™#¿Ú¡5Ú­` ¿ÙWQ †¾¿Ö4;‹ú¿Ø¦•€…K"¿ÞAÒ½ý|AGNbll3FGL J0054.8-2455FRBA J0054-2455?ïþθ<ûg?µ,™Ø£?#|0I–C?µ,™Ø£?ïêœt¦E?qg¤`fW?ec‹¥ÃŒ?qg¤`fW?ïõŒ¤òî?V[S2¡?TæµÎÒå+?V[S2¡?ïô—lÖ6?A?Î)?VÑ(NÅ4N?A?Î)?ïý/Ífê_?*Çi5µ={?6"‡Î
?*Çi5µ={?ïÁa™Íñæ?…'ÄK;@?O3#Uá?…'ÄK;@?ïñt0öS?jKX7¶e?]ßâ
5?jKX7¶e?ïև˳??e¸¶q¡?tý<w´¼?e¸¶q¡AGN4FGL J0054.8-1954¿í+¶F©ÀT¯ƒÏ,ù]À;V¢¤V§À<³6z—@·"6Æf@ÛeìÃã?Ë8àä›v?²'xÛJ?çy>@Øb@q¦KÝ«?ïú;Àu{'¿áZ³À6fn¿åôIÔ_h¿ã=ˆÁÛC¿êÃ
¬+l•¿ïàbb ´AGNbcuTXS 0052-201?ïþ¦ø?àMˆRâì?'wQŸ¡?àMˆRâì?ïðdœaÊö?bœ5Âçì?_6Æÿðóî?bœ5Âçì?ïë+µ:‰ê?X«¨ÿÙå?dÔJâRÎ5?X«¨ÿÙå?ïûÅjÁk?(äÚ¹N£?@êWÇÃ*?(äÚ¹N£?ïþèŽ|ã‰?Ôbׯ?!wm†lž?Ôbׯ?ïÃÛ»8a?'»+ZcÞ(?~"Zàƒ³?'»+ZcÞ(?ïç‰Ì?o'"ËûšV?hvðϙÜd?o'"ËûšV?ïïGÀ!Ýd?QBêÕÞ-Ç?`¸?´çL?QBêÕÞ-ÇAGN4FGL J0055.1-1219?æ¢RÄYFÿÀRʯáÚ{À9ýÜ-'àBÀ<m×ΈŽ¯@¼p¬'ð@
'¤Òh?¹ãD![ß?ÀÞÏ-Ðã@F{¢7ÍÍ@2"iY
?ïç«?´Jö¿ÝA"ßþÙ¿ã—všÙ5¿åüŸù/+¿ëC0×8`š¿ïÿÒkÀAGNbcu3FGL J0055.2-1213TXS 0052-125?ïü¬Àà&é?+†ƒ•¤BŠ?:™úd =?+†ƒ•¤BŠ?ïï®__0?d­o³ÅÖk?`Q q¨ ‰?d­o³ÅÖk?ïÅo_Ö¡¯?}…^™~nØ?}HPqX?}…^™~nØ?ïü#îácw?)m¶ëEøB?>àŠù©ˆÕ?)m¶ëEøB?ï÷
­Ýã?L×Tg¼ò?Qëò.ª‡?L×Tg¼ò?ï¸ÈØ?‰¼ê?ÍÉ·š'¶?‰¼ê?ïmù˜1å€?Iö´ Ý»?'@Ìþê¹ï?Iö´ Ý»?ïöÌ=ìÛÇ?Bïõâ=ùë?RgƒË'Â:?Bïõâ=ùëAGN4FGL J0056.3-0935?Ò0WjcåÇÀR¸ºÇËÀ9}îþOü˜À<÷FóÚX@ù¹î"ÝÑ?ýÑ–^{¶?°_˜kòˆ?|OðŸ%?ÏÝ=ëô@÷ü\‡jm¿ë' À¿Î7¿ÓƼgyâ¿àÔÀ·Ô£¿Ú:@m®YD¿ây…'`lý¿£\»~óAGNbll3FGL J0056.3-0935TXS 0053-098?ïÿï	ÒV?å›ç»n§?¢!Ëð?å›ç»n§?ïóuæÛA?`VWR´Ç?YÄiC>?`VWR´Ç?ï÷!E[:?U:{R›Ô?Q½uˆÄ'r?U:{R›Ô?ïýœ.Z—Œ?$.f íþ¥?3ŽÞ«´B?$.f íþ¥?ïþy(qŒ? =Ýo†?(m{È*›Œ? =Ýo†?ïÁ섫©o?†‡"&N&?	½›¼ì}?†‡"&N&?ïö«ÍßØ?hÛ—`Df?S¨ɯv?hÛ—`Df?ïû^ó!íˆ?9ò!–5L?B"3sãùµ?9ò!–5LAGN4FGL J0056.4-2118¿çñKJ'[žÀUþ!ÙnœÀ9Œ Á@§À;ý˜K$Â@"żãÊ?û·ü«·©O?³+»Æû}?¿›?¡€˜Â@Œ˜¼úDz@	Ê'§…?ïÒ"4ÕË¿Á9‡ ÄÌ¿Û<á²·ù¿ÕŒò3Ž£¿áV:¿n•_¿ìcxt…äAGNbll3FGL J0056.3-2116PMN J0056-2117?ïûô%3ô­?<‡†æÉV*?@/k¡ùõî?<‡†æÉV*?ïâþ]Ï¥+?sÃñת=¯?m¢,;Mƒ?sÃñת=¯?ïÅòqÞr?ØEM}f?}ñNŸêÓ?ØEM}f?ïÛìõX©‡?XŒ`Yß«?r	…C-µ?XŒ`Yß«?ïï%Epá?^
Y<2¾u?`Úº«tþÔ?^
Y<2¾u?kœA{?"
Xý²?‰ÐeÁ•a?"
Xý²?ÉbÆ??*­ë›?¸¼yBŒ??*­ë›?"óÆ?zjf^Wpú?×úMDž™?zjf^WpúAGN4FGL J0056.5-3936¿ïÝ?¶¤AhÀS^/@_k À<6ë!LÀ=¬Âý@2@½}9;¶@%1ÛD^Õ?ܪâ`?ï«W½V@)x]@°Ac¢'»¿ïûvÞ®¡"?ïÿ™=SG¦¿ÄOF,Š¿ãuC
›Éö¿ïÿ¾AÏ?Øх™1"ÎAGNbcuNVSS J005620-394144?Ꞙ°KÈç?ι˜¬M•?Ņ>ÐÜb?ι˜¬M•?ïmÛƒT?¤ƒí¨íýý?'DœÀ1p?¤ƒí¨íýý?êåìZŸò?±-ªš¡@'?ÄhN—€7?±-ªš¡@'?î…y‹©ŽQ?"?ž$A?§¨gFCô?"?ž$A?éëÈ®MR?ÉOÙÀ-á?ÈPßùFÊ·?ÉOÙÀ-á?ë÷Åü-ã?ǎxœQo?À ñèHr?ǎxœQo?æX£7ۗ?¸ê—0ZQ4?ÒýN¹HÒ?¸ê—0ZQ4?çaõÌÜxM?º°§¬p¥ž?Ñ<fGg?º°§¬p¥žAGN4FGL J0056.6-4452¿¹ÂN<РÀRg ù	lÀ;/­¯ÑƒÀ<ÆuŽøUè@ˆfed³´@½ãÖÕ?Н™šäó?Çj½m^R?ò‡'Ñ(| @"'R"aª?ïþ·€ŠT¿á3A
ŒJü¿á*XÎÎ.Í¿ë)«Êô…x¿ÙccGP!¿ïÿQ"W6AGNbcuPKS 0054-451?ï±H.íÔ.?ªÖd3öT?ƒ­ô9Œ4u?ªÖd3öT?ïðº×Â?en²+áH?_ȋ‹–?en²+áH?ï¤$qU²?'AW¥6½x?†öã»j"‹?'AW¥6½x?ïö/Pih¾?>½ñ±<å?S¡_á³'?>½ñ±<å?ïð–*¤Cl?c-ÃÐ)o?^Óª"½8¼?c-ÃÐ)o?ïÐˈ+?} «YQ)d?wûšYÎΓ?} «YQ)d?î"uß;uˆ? 
2é6e?¦¸¢Ü\z? 
2é6e?ïÇW+yÅ-?o»²ü@z?|Tj4¯
º?o»²ü@zAGN4FGL J0056.6-5317?í3[½sœ
ÀOèMüãÀ:ïiÓÀ<ÔüA.žy@õPŠ\õ?ÿÖt|?Íü´Ük%h?É-´C>??ûG
‹ýá@n³}ÆTc?î9•"zœ¿á,c5Y~!¿â²Ÿúܪ¿Þts®M†¿æ̚wåê«¿ïûç6Û^`AGNbcuCRATES J005630.93-531931.5?ïþ¸E<†?1qVY}ö?.ôz&i'?1qVY}ö?ï÷ÇX³d5?S4MîA?PqN¿³61?S4MîA?ïèçK9u~?ce+HC=Õ?g´ÉJ2:?ce+HC=Õ?ïüÿ©‡½?!]0pCL?8²b?q¤?!]0pCL?ïþ¬`È?#,òAa¾?&õ6-õ»?#,òAa¾?ïÜLõ¯¢£?rÖ­È
0?qمf?rÖ­È
0?ïՕ´:bZ?5ß°¶3?u5%× '?5ß°¶3?ïøùåÎjK?;ÝÍj$=?LhÊ/ÿS?;ÝÍj$=AGN4FGL J0056.8+1626?äȱÚ$›ÀG5HUÚ'(À:úÀ%zÀ<ŽOÙ\'@Z%"ü|?ýÔ§Ý);c?×spºþI?ÍËù'ɝ˜?ó«¿¼CÎ@Ÿ''À1?ïԘ"¡¸¿è¸¸G¿ã3Ìý¿Õý-};¿õ¿êÐà"&þ¿ïþÈþ3:AGNbllTXS 0054+161?ïîÝ+G_?T$3jß÷?a"ÔÂ?Ð-?T$3jß÷?ïï‡|-?a6|Ö϶à?`àx«®^>?a6|Ö϶à?ï±Ë¾'?{ûWE?ƒ`¼T?{ûWE?ïáø,™]?Pë{q

[?nÓ]—?Pë{q

[?ïë/.Òâw?\gj1ËùÄ?dÐÑ3üÁ8?\gj1ËùÄ?ïÂŽ¥Ÿ·?"IÐRÆ%?~þ¸›R,y?"IÐRÆ%?ïLVòÍ^å?'o¸Gû.o?–u!®ë)H?'o¸Gû.o?ï£]gî§?swóuãø?‡(¾ØEæd?swóuãøAGN4FGL J0057.0+4101¿œ¥È»•ùÄÀ5×qûÅޜÀ;RÏè
?õÀ<Å ªšrÝ@ '¶%–h?þöêB(™|?ÎxADÃÔV?È#ýu·O?ö'/ðˆ"¸@²æ˜>%¿ìuŽŒö(¿ïþÂé<+?ïú½ÖÄ.¿çÖBL*Ñ¿Ñ;\øSŽ¿ïÿŸ‡ð#êAGNbcu87GB 005415.3+404404?ïýU†¢Ï?-â#^þ<·?5SËS'á?-â#^þ<·?ïôÀãÉz?W+·ž$^R?V~ßÊy?W+·ž$^R?ïâ
ÍYJÛ?gNÜfÍj?mò2Ôü•?gNÜfÍj?ïõ}ǚ͐?Bó\3¢ß?Up'íY?Bó\3¢ß?ïý¨ZZG'?./¼™Ž«#?2½+Ž)>W?./¼™Ž«#?ïÔ«K{\?x)ù*PD?uªZ5Cl[?x)ù*PD?ï½…ü?ÆG`ˆt7?€¸^ÎÕ?ÆG`ˆt7?ïßSy=^?g Y¥+~Ï?pVC[ì?g Y¥+~ÏAGN4FGL J0057.3+2216?ã;e¿ÞŽÀDIúÁҝÇÀ;®ÈÕÇGÀ<¥h[3,@¬ñ\y'´@G•övêB?Ђ§z,ìÈ?ˑb"së?øŽv pMp@‹ND†˜?ç{âN"8¿Ñ!Åâø³0¿ÛK·c"ä¿æ#ª"" [¿çñž¨ÍD¿ïøuÈ9pAGNbcu87GB 005452.5+220227?ïùLhœ»?BÒ>ÛJ?JϾy–¯b?BÒ>ÛJ?ïÊü=?bæ"ŽÁ="?a`B`þ›?bæ"ŽÁ="?ïØZo7Eg?hqó—M?sÒÈLÿôØ?hqó—M?ïݪh,\?PwsÈ
?q*ÿ>+bC?PwsÈ
?ïø Ǐï?M<ÛüoØ2?O|â·'«?M<ÛüoØ2?ïÅNˆpžÆ?7Ÿø?}X»Öøñ?7Ÿø?ïf¡¢Q¤
?#Zßé?"+˼ª¶e?#Zßé?ï€`›~Ô¥?u£ÀëiYY?çÙ'*½?u£ÀëiYYAGN4FGL J0057.7+3023?Ü­eqáUÀ@:2 f<uÀ:]á‰ó3iÀ<qƲ˜¬@à[À6ã@/¿üñý?ºW¬5Ów¿ù/£©	q?áájžYqá@h…2`z?ïÞßY—K¿ÚßùD¤õ˜¿ç2Ö·1Z¿â·U¼®¿å"÷¡aº¿ì\8åú›<AGNrdgNGC 315?ïûB¾ÁqO?1ηrw:'?BõÝ­ã?1ηrw:'?ïïȒ!ø?b¤´FÅiˆ?`ñ7Šº¿h?b¤´FÅiˆ?ïà+Êð9ö?jú©ó¶J?oÔ5%Êa?jú©ó¶J?ïß·Ã{?f?RõO~Áœ°?p$T>D®?RõO~Áœ°?ïô6âÙî7?O¢#ÅóºÛ?W':…Ý'?O¢#ÅóºÛ?ïÀtۅ]‰?Š*^é¾vÓ?Œ.2ó¾?Š*^é¾vÓ?ï½s•›T§?€	ìÝuPä?€£šŠ®8?€	ìÝuPä?ïkb-éêŒ?zŠÆxºóÒ?'"ºI¡æm?zŠÆxºóÒAGN4FGL J0058.0-0539¿ÆÉ'?f{ÀQ1&éyÀ9àL'ÿzÀ<>$ìz@Ž¶çˆ:@Œ_|gY«?µ¹f"‡Ý?š%™¼Úç?å·;"@ßÅÍÕ¿¼o¿*¢Àà¿äu0cu^¿çéâ‡I5¿àïâEÚÕ¤¿ð?ïÿÿ" 5•AGNfsrq3FGL J0057.9-0542PKS 0055-059?ïûÁ'¹=µ?DNjލ&œ?@û`f·Fž?DNjލ&œ?ïò3¶‹‡?`…Ú8‡é?[™æÌ¢bo?`…Ú8‡é?ïşn0y?LŒ~˽?}0v­jã¢?LŒ~˽?ïÿ*ý|'?äÑûC×? Qªµ?äÑûC×?ïü·›.¼x?>{'/¾Z¤?:C%1ö'÷?>{'/¾Z¤?ïÄjH{Í^?ƒ¸úý¨?}ÊÛ m$ô?ƒ¸úý¨?ïØ -z•%?xú'ߎ?sïé%ص™?xú'ߎ?ïýVQ'¼'?.‹whÎ?5Mt¿˜Ö?.‹whÎAGN4FGL J0058.0-3233?앒Ïâ>ÀU>úç'À9?ÊKM
À;ý±Ù+á@›4
MÆ\?þ§"Ô@^•?±MŸ^ï=?ÃüiÈp@ÒàýÜ9Q@Ãö9'­š?Ì♨28·¿ÚtØdZ…¿ß´© !óñ¿â—¤—#"¿å_‡dU¿ídÂw^[AGNbll3FGL J0058.0-3233PKS 0055-328?ïù
=Vß?O	 ¢-ƒ?K‡×Éhm|?O	 ¢-ƒ?ïñ…@œ'h?a='¾«bI?\õ~AÈ?a='¾«bI?ï:òÍ<‰H?"®cƝ	›?˜¡¦O×Ñ?"®cƝ	›?ïónFڄñ?DÃÆí¡?Y#qû?-í?DÃÆí¡?ïÏñeÍ(?xÄÓGOö¿?x~‡7ËØ?xÄÓGOö¿?ïËîÕ؆Œ?{V«Žªð?z•+þ?{V«Žªð?ï'¬'¡ì?˜`«hP?œ
uäX'?˜`«hP?ïÁx}À??n¥kV´›i?CÁ;m@*?n¥kV´›iAGN4FGL J0058.3+1723?í‰ëÀÀF¹àÞ҈ÎÀ;ײˆä@À<àòŠÌw<@"\øžC"?ö¬ôI:Ü?ÙWM¤xšÆ?ҏ4¹¿ª?ûG&Ɖ½@1ƒ°¤"¿ÎЈgB.¿ï¼ÚF2y?ÄO{τ7?ÛbY&D¿ÕäŒq'êS¿Ó]$É8AGNbllRX J00582+1723?ïü)—[¯\?0|ò/Pt®?>³CfQ=P?0|ò/Pt®?ïñJ±A'?_J'hYšû?]jœõz[2?_J'hYšû?ïÖ8€qvÝ?q¶¦JMV?tã¿·v]"?q¶¦JMV?ïø•òt*?>,u£Zž%?M¨8W>Ï´?>,u£Zž%?ïümî°?8ÂÖĘ??ԗ‹"AÊ?8ÂÖĘ?ïÃi–òuS?Ñg{ö€?~K4¤Qúc?Ñg{ö€?ïç>é}e9?p¤¨˜?hÁºô^"?p¤¨˜?ïã·UIç?hxŒîåJ?lHªÎÖ(t?hxŒîåJAGN4FGL J0058.4+3315?ßóTïN4ŸÀ=™-ÛÛ]‰À:ŸZ±&~À<ƒ3ÆÖé†@¬nëÆ>@iød*L?Ťò}¶d+? zƒB®êþ?Ö¤b‰·ú@M™»ÓU¿ÚWvÿÄ^¿êxbý¦3†¿Ü›aÅ¿ã½#â]¿æÖ©ZýV¿ïÿ¼ä!}(AGNfsrq3FGL J0058.3+3315MG3 J005830+3311?ïþÇ'5<è?k*8¯ô?#ŠÚ$?k*8¯ô?ïõ2×=W?Y¸>.Î?UšQ"òL?Y¸>.Î?ïì(R??kLê׶H?c×­¾y ?kLê׶H?ïÿ­õœ#ã>óñÄXÔ?'–C§æÌ>óñÄXÔ?ïÿ
ÉK|Å?ÀØ›#û?¦Õ÷˚?ÀØ›#û?ïÖ»ôÄ?x½¸JE[Ç?t¢Øòg?x½¸JE[Ç?ïë—×çKî?sžÏ^¢!?dh(*4?sžÏ^¢!?ïÿi|<ÞÐ?²jĤ/?Ð~xú ?²jĤ/AGN4FGL J0058.6-1140¿èÊ5ùêšÇÀRiÂ;ySÀ;Tük 	‹À<¶g÷`N@¡'ðµµ.@Êyžø?Äqw¼zL¿£ð ¢³"ã?۝i?þÁ¶é¶'y?ï¹c<{¿ç³ì+7¿ËÑþdõM¿èõ¿Ÿ½ 	¿ÕAé"h"ú¿ßÒ=ºu²4AGNbcuNVSS J005832-114050?ïýŽ‹Û?)%$%i¤?3‹¨<õ:?)%$%i¤?ïíÆo: e?g¹"L»Wu?b9¤c[I?g¹"L»Wu?ïì‡FÓ?Xeß3Õæ?câx¾¬Eg?Xeß3Õæ?ïøôcû¹0?4F·‹Œí?L.obH¼?4F·‹Œí?ïû§0¹Žà?7%:ˆë¦?Ac<¹pZ?7%:ˆë¦?ïÁµüjŽ?" s¤þ¬¸?%Å9žõ?" s¤þ¬¸?ïåyC/L?qœxLº?j†¼èB'?qœxLº?ïÝßJÜP?d¿
À1±Ç?q|qï/õ?d¿
À1±ÇAGN4FGL J0059.2+0006?«žØu[þ'ÀOXn¹ªÀ:Ôf_°iÀÀ<g[±×~@ðü@\†Ô?Æ3°†›;?!ßÑa\w?•GÒ¸°Fk@Ê}ª{¿ïûSþ"Õ½?ï"'úñ¿èýk@íù¿Üo<"ððÿàÄŠ]¼t¿ïÿ·¼]êAGNfsrq3FGL J0059.6+0003PKS 0056-00?ïþµ&#;?"ë~Èñ?/D®}ӆ?"ë~Èñ?ïñµ›z<?bq™¥
:?]ҔJ™é
?bq™¥
:?ïäûý¼Ù»?h3ŸÌs?kƒ¾í
?h3ŸÌs?ïûÄ®40?*ó[Ñ…?@íGÅ×ó?*ó[Ñ…?ïýº'?*x:·lôÔ?2+sù-r9?*x:·lôÔ?ïż¥bO«?"ä1õæï?}!­2«^u?"ä1õæï?ïı¶NŽ·?ÐX1É?}§$ÅzÔ£?ÐX1É?ïë<½(G¥?X­ðOF+ä?dÃB"`ú?X­ðOF+äAGN4FGL J0059.3-0152¿Ôÿ§aû•ÀP+±mÀ: ö|ÉÀ<om"BJ'@!1‹¾9·?úJ"H)d}?ÉT™_b@?À:îéWG?öäŒ×ê7@w¤!¸?ïNëUN.¿Úb/ »è¿ëM&ßgÚ?Ù>&@Üi"¿Þ‡j'̔¿âqÐý³õeAGNbll3FGL J0059.2-0152RX J0059.3-0150?ïýš7×»F?.d¡LeN?3.Béu®:?.d¡LeN?ïí§[VÆi?e֊ŠåÑ?bX¤y`?e֊ŠåÑ?ïç	sq<?i'ÒÅ})Ï?hôö¦«Ì?i'ÒÅ})Ï?ïò³™Jt?C…ÎÁt
Ž?Z˜ÍŒÕVÚ?C…ÎÁt
Ž?ïðýGWÇ?`÷—'ç?_Ü !i?`÷—'ç?ﺋ@)T§?ƒWº7?]/ê¬V?ƒWº7?ï¨ÎÈFø"?‹DÙ´øÖÒ?…ÌMÝÓ?‹DÙ´øÖÒ?ïϘ¨@5?k2@«&l?x3¬Ím?k2@«&lAGN4FGL J0059.5-3512¿åÄHwúÏÀTnñVIÀ;-‡˜æsÀ<×hL´@ '¡R Œ?øàLÜQ¥?ÔÓ)=+Ç?Ú·æ@'?®@ºQÎ_@'.¦[žâ?Þ÷~°4;¿äRKý."h¿Çáä÷eý‹¿ÕÝmCzS-¿à_'¡Û\ˆ¿ïüjÿÓ4pAGNbll1RXS J005932.3-351049?ïûŸ'2öU?:¶ÿS˳#?AºË%ω?:¶ÿS˳#?ïò,µ7?böû#Á3
?[§Üpq®?böû#Á3
?ïÂÅÔØVe?xÏÀ¸èww?~"ÔÍf?xÏÀ¸èww?ïôDøI¹?@ÚKðòžï?WwÃÍt
€?@ÚKðòžï?ïü¤1M*?9v§†Q??JߗÜÙ?9v§†Q?ïÓAmÞÓ?zg~ÛÒu?v_I(ÍZ?zg~ÛÒu?ïÅÜ|±ñ?Ù­ó#;Ú?}Á¿·Ï?Ù­ó#;Ú?ïݐªeLi?cŠìUDÕC?q7ªºËçÎ?cŠìUDÕCAGN4FGL J0059.5-3338?éþ¢·œÜ<ÀTÐwpyåŸÀ:îßDž•'À<}þæ$Œ§@ÀQ>@s³{j?Ä(3e]&ø¿Jèåë‰?Å|ÔýGéÏ@8WÁÝÛ?ï€wSôsÛ¿çՊv'•¿éÈ	ïm¿å
@Zc"å¿îâæů¢¿íå¿ý±q'AGNfsrqPKS B0057-338?ïú
?BÑ/RŒ5Ä?GÔDÀJ!…?BÑ/RŒ5Ä?ïòÅ#­{›?cî=§Yæ?Zu¸½Åù—?cî=§Yæ?ïÞϳ~iŠ?fOf¡?p˜&T	
û?fOf¡?ïû0)}A?/^à´¿ƒ(?C?ÆP'È-?/^à´¿ƒ(?ï÷ÞßÛ¬?R/{sãÚ_?PB@>o+É?R/{sãÚ_?ïÓØÚ² ?}OËn?v'Ô
ˆ4?}OËn?ïÜ'?"ï]?wÐg?qì`5b?wÐg?ïã_æ
ç?^LètsÉi?l ÄVñ{?^LètsÉiAGN4FGL J0100.3+0745?Û&™žïfLÀK…}™ˆÓÀ9À~à°¯À;¸ ؽ›×@~DzƒSÝ?úñ`åóå@?°'IïgÂ?Ãahz½¶Y@Y…ðoiD@
õöA:\ó?ïãqߖS¿¼j»_¼þù¿Ôþwštá¿Øót ¹3¿áÏû'½¿ëÝ­Å ‰AGNbll3FGL J0100.2+0745GB6 J0100+0745?ïí=×7E"?us˜_ÔA?bÂ(ëõ÷?us˜_ÔA?ïÖóÀû³?}X?Z?t†r$QšZ?}X?Z?ï;P''r?•Fy(c`?˜•û›©½?•Fy(c`?ﮆvãGt?n™èXÍVJ?"^bF~7?n™èXÍVJ?ïoÚC‹x¢?'œ>'?•Þ?'·ŒÙ¼?'œ>'?•Þ?îř»,Ã?·ÍSKÕ·?£¦dP‰Ë?·ÍSKÕ·?îÀ¤˜PCd?¸H7O˜1?£õ¶zâ¼?¸H7O˜1?î¥|‡Ð?'(ô$†ph?¥®ˆA—÷?'(ô$†phAGN4FGL J0101.0-0059¿íû͍´UÀOáXâe,À:봙Р>À<[‹)"N@•)œ±|@mFTx'?Çö¬m±´¿"o:Æy³?¿D"Wá@àG
€Œ'?ïQSµø ¿ìŠ…à)Jý¿âÛȳb˜|¿ß㲁òÞÚ¿çï\¿Hª¿¿ïþÛ<ÒfAGNbllNVSS J010058-005547?ïývÌα?(eæpƒ<?4Ižça'j?(eæpƒ<?ïñH's"?`>ó(SͲ?]ùo(E?`>ó(SͲ?ïêý‰zŠ?qf2üæ÷Å?evG?qf2üæ÷Å?ïùI @£o?0͏¼
…?JÛ~ȸþ?0͏¼
…?ïùT­ßÕF?O´•È_)–?J­I
ëB?O´•È_)–?リ¨"?‡%N÷'{Ì?€YøȔàø?‡%N÷'{Ì?ïÞcí²—å?xœTù%l?pÎ		'iÑ?xœTù%l?ïä=lÈ?X¯7ÚǕ5?kãþ¶4 ?X¯7ÚǕ5AGN4FGL J0101.7-5455¿Ñ5G×Ò\ÀOÅ?9ѳÀ;»¸¤÷›­À<ùÓ5@"CS/ÒÖ|?öÔxwàâ.?×?=ba(?Ér0‰Š­Ã?õ©óƒðºé?ùÎ
"Ñ¿ïì'œ<Œ?ïûÌ>²mP¿ä#%  ?͗J	
šÈ¿âê¦gv¿±X•~̺AGNbcuMRSS 151-121576?ïý'.S`¶?+ä(揻?6ƍ4™fâ?+ä(揻?ïð#•¹;?dgÌn`af?_¸Ö"É4?dgÌn`af?ïÑÝ]Ç9?sõøŚµ?wQ#ò˜?sõøŚµ?ïòHC²ÿ"?J7‡±}E?[oxRˆù7?J7‡±}E?ïýWÕ1¨Í?1(_ó@6?5AXh.?1(_ó@6?ïÁç^—–?‹µŽèq¶)?Q±?‹µŽèq¶)?ïÇ@ VŒª?~?ˆjÂø?|_ïõµë?~?ˆjÂø?ï¿(aªÚ?u ¡Ú‰?€5úªTù"?u ¡Ú‰AGN4FGL J0101.8-7543?ì^ˆ!³?CÀD°p~]À:øóºw_³À<drû ï@ú}µ'@'°¤xí?Æ0A¦¾p>¿©cKn?ÞÂ
y?ý$2³=Û¿è,ÊRŸ	¿ä œiàn¿êÙCӔg¿ç"\¾që*¿ïôL¾´ ?ïÀÃþ¬CAGNfsrqPKS 0101-76?ïóNHãHº?'•|?YcnZjËv?'•|?ïè(nÝQ?yÌ_Wg¿?gג(Ü*?yÌ_Wg¿?劣— V?T…ÕJ×`?†X¿'ÖZV?T…ÕJ×`?ïù@ýºð?;Ÿãʒ"h?Jü
02R?;Ÿãʒ"h?ïùŽyAÏ?WLbÃ¥õ?Iǖ"†\—?WLbÃ¥õ?ïrøÊÎè'?£çÔl×®M?' æ©'—?£çÔl×®M?ïŸJžê	?‡&·?jû¬?ˆ-XˆQ•?‡&·?jû¬?ï…T_äÓ?†,¶Ҁ?Ž¸ªòUŸ#?†,¶ҀAGN4FGL J0102.0+1639?⎯;}ÀGRv‰ÊÀ;IÍ©kŸÀ<–=u¬T‡@' 'àð@P'Û_6Ç?җýãA?ÊY ãOp?óñIÈ î@ÛR¼ev|?î¥k¼½¿é"c!7ˆ-¿×»d$lÆӿ代yí+è¿ÚÒ¶Ù ¿ðAGNbcuTXS 0059+163?ïøU­Ë]?Cúï™|rÍ?N«Æ6Q"©?Cúï™|rÍ?ïñ
ÿ¸\}?_ÃÐ]ö·?]ê
¸¤ž?_ÃÐ]ö·?ïÖNyÆќ?sՍÃÓûÿ?tØÃw©Ý?sՍÃÓûÿ?ïõ×H·åñ?8¢'5 6Á?TQn⪽U?8¢'5 6Á?ïúÐã8<?@P³hî?D¼rdúV'?@P³hî?ïȼÕ2÷Ï?_‡K?{¡•w²$f?_‡K?ﮍx	b;?"£!š¾ä€?"\¢.³Q?"£!š¾ä€?ïØøaœæ?aö¸‰kõ'?sƒÏlâö?aö¸‰kõ'AGN4FGL J0102.4+4214?ë gã¨À4–™Øƒº4À9°²2í"À<Nõw/@îȎ¤ž@û–¼o‡w?´æ&eŠ@?ÃÒr¾Žpœ@'3cښì@¨§óúc3?ìPSà뾿å¸Â>SwÌ¿êiˆ†a¿èÏ{5U¿ç'kë
¥u¿ï÷§pò±AGNfsrq3FGL J0102.3+4217GB6 J0102+4214?ïý•í£Ã?5Qv*hk?7ëQ16Lg?5Qv*hk?ïõÔ†îá?U(?90?TWҁo×?U(?90?ïŊ`–˜³?vtì哼?}:Ïπš;?vtì哼?ïý-k"C­?"ÓßH"?6"£íG<€?"ÓßH"?ïü°®oOÕ?@@áï"b?:zŒ¼{×?@@áï"b?ïÕm"K]?yp]?&)?uIuOÇmY?yp]?&)?ï ´Ê'M	?"BnÔ7éë?›éf­Ö^é?"BnÔ7éë?ïöTëH«?CuˆE‰ü?SV*êJ?CuˆE‰üAGN4FGL J0102.4+0942¿Ê¶¿$·WÀJˆÝ½µØ•À:áüëx‰À<i
fL@ Ά5•8?ûþ·Ë³È?ÒO)~(¤å?Âå+é<ïõ?íúö -G@ãñ@J¿ïêÜ0?ï>ž¡@¿êáz~vR˜¿ºÍ¹†ÉÞ0¿çł Ù©Õ?vCA"jïsAGNbll3FGL J0102.1+09432MASS J01021713+0944098?ïÿ:Éxô?m§Ì©›÷?¼Ø¹¿?m§Ì©›÷?ïð-9Ÿ?c7OQÞ³?_¥/ãNm?c7OQÞ³?ïÅn̼[»?€×àF:Bº?}H™…Îy?€×àF:Bº?ïöç'R!­?=D·SîcX?R0ûS}•?=D·SîcX?ïû[Þxï?G0…áT?B…è
Èq?G0…áT?ïÅéúì+?<öþì?}›ÈiW?<öþì?ïK¨áqZÇ?–D3ëÒ¼õ?–Šãسß?–D3ëÒ¼õ?ïÙ"бÖ?hÙ»G¿1Y?sn—·"?hÙ»G¿1YAGN4FGL J0102.6-5639¿ÉÕRWeÂ}ÀN3ք³žÀ;¹¯¹–À<¥}xÑ¢õ@ 9†˜*?ÿ›øԒ"ì?ËÞs'êÕ¡?¾Üö êAŽ?îÞx@ƒ}Î@˜ªøè?îÄ8ÿzôé¿ã×ÓÐw¿Þ'•ðŠ¿äþ£%3–¿Ù߈'3™‹¿æ›Ãu56CAGNbcuPKS 0100-568?ïþÏýur?0hjø_Ô?#C»t«?0hjø_Ô?ïö³-ç¼?R§¢¢`¦?R™á\¸§ü?R§¢¢`¦?ïô–½œ-H?Y‡5 —+?V҄d°±?Y‡5 —+?ïü nNV?%Ž¥ÔIEª?>üŒáp?%Ž¥ÔIEª?ïþ†Ï?$i'°n?'ŸäÀ??$i'°n?ïÝWöÈ/?r'8™?qsÔÚøj?r'8™?ïóÃq·ÛØ?e¡­‹Œ»?Xy›GÜ?e¡­‹Œ»?ïðó‡é?OßëíWž?^øä'¾R?OßëíWžAGN4FGL J0102.7-2001?ãòR<ÊÀTœWS£ìÀ;öÚó=À<ë…à1@"m.B]ž?ìHBŽðÉ+?è?àáVÈ?åÁ=¢wä"@¹`ß=è™@f±?R¦@?ìü辚Úâ?ïšÜ?0—x?® Æßwõ/?€3
.ÍÙù?Ɵ­¯Ñƒ¿äè/(âwYAGNbcuPMN J0102-2001?ïúí‹Ö"Ô??H4±'ÈÑ?DIÑi€??H4±'ÈÑ?ïî&WhØÃ?l¬V|?aÙ¨´õ"?l¬V|?ï³øƒÆì?uÛ*høQ·?ƒß	W›?uÛ*høQ·?ïùÜEC^­?@A8щ¯Ü?HŽëÀ­Ú™?@A8щ¯Ü?ïöÆÝca¾?MÄH‰qԊ?RrDÀJD´?MÄH‰qԊ?ï¿1¯-2F?…;ö‡M•?€3"+Är—?…;ö‡M•?ïÌ9J_°Ñ?}ßèZ_X"?yãZêDŸr?}ßèZ_X"?ïö]@>ú?Wÿ|ðva?SEÇO?Wÿ|ðvaAGN4FGL J0102.8+5824?ÔÕ$qpÒóÀ·ê¢ ©XÀ7Ü.u^PîÀ;GŽd²1@@6†@¾‰Þ:³Z?—?úØÍ?°©G¢'@4XÍ!@ÅéôZ/¿¾ÖK¦œŒ¿Þóc9‹<	¿ä->\\!i¿äpˆÿ¢´¿årðR
¿è(ê¿üÚ²AGNfsrq3FGL J0102.8+5825TXS 0059+581?ïü)v›è©?8'ÎM—?>´M(Ì_™?8'ÎM—?ïíó¨?pŠ'ñ³ü¼?bç&q‰P?pŠ'ñ³ü¼?ïÝV¥S63?u\9ÿ€S?qT­:8±?u\9ÿ€S?ïÿ£ä¡)Ü>þªjañ?ʦ#òi>þªjañ?ïýúd¾#D?&3÷Ÿâð?0,Û%p?&3÷Ÿâð?ïŽA¢?c ?¬\8«'?Œo—}å§ó?¬\8«'?ïÚ@wO˜?~D)pSà?rßò¼$*?~D)pSà?ïÿdk([Ù?v6)	×i?r"í¯??v6)	×iAGN4FGL J0103.1+4954?æ)³»¦+À)ÖV%¦'¶À:o¬)ÜrÀ<
(¼·«Ó@M"àú+@Ä>š4?ÆíG@±K?¶zPÑæ?ìàÛwŠ{@×o?t¿Î£ –x|é¿äœG(³}p¿é½Ê›š$Ú¿æö#l¿êCá9Ñ]¿ïþ{€©Þ‹AGNbcuGB6 J0103+4959?ïôÂm´t¢?\/ÅO´'?V{$¤Õ*ø?\/ÅO´'?ïëð13‡J?n›ó5ù(y?dÎîÔÎ=?n›ó5ù(y?ﺵ¢Üð?{I¢ù¦1ö?R—WÅÎ?{I¢ù¦1ö?ïÚO]F"I?U¤sôå·?rØQIx‹Ù?U¤sôå·?ïÞÝnc=›?r^EEZƒS?p'HÀ¢ÂÄ?r^EEZƒS?µÃ-?'Ë·`ðSç?‹Ғ¯P­?'Ë·`ðSç?ï-Ëeé?"×½Òō?œZF¤Rzä?"×½Òō?Ä2R?')çfnº?§5ƒ¹kB°?')çfnºAGN4FGL J0103.5+1526?ywÇÁ°ôÀG«ò<ÈÞÀ:ëCø}T¿À<^1
¿@å´ã¡ûh@ʘÅ^C'?Äé)yËóß?œQö†žY?ÕõèúÕÉ¡?õ­:mº¾¿ïûœÞÈwÓ?ïÍ$Á*'5¿åÞ¿þÞ÷¿ìÄ9ë´¡¿×ãJ<º?¼ŠC:gZAGNbllTXS 0100+151?ïþg¹o`?*ô:·zlæ?)"jMBS?*ô:·zlæ?ïâ¯[¼ƒ?vQ6W˜«Ó?mP¤eÙj?vQ6W˜«Ó?ï''àCÍ	?ŽºkÒ~@?vò|Y¤?ŽºkÒ~@?ïç՛õ¶È?TÜ),èJ?h*cýêŸÆ?TÜ),èJ?ï÷ôq	5;?M©ñ£p@?PNWUI?M©ñ£p@?ï^Ž‹ý|?¥\ŸÓšq[?"..ƒÏlŠ?¥\ŸÓšq[?ïbS'"v?'2Õ©D{?"µ›¾':?'2Õ©D{?ï$ÎҜ«®?7i÷á´?›f%§C G?7i÷á´AGN4FGL J0103.5+5337?ãm!Zå÷
À"gòä¼®À9¼ñÈ.Ø[À<!ƒÞFr@ y:æ/õ;?ú	»…|¬#?µ÷ÝòŽþ5?½³ÃçJý@ƒZ'ó@Þ¿¾qj¿ð?ð?عÚÂ-âf¿Ø("C2¶¿Ü¾ƒžZž‡¿Ú(ÔɎÕAGNbll3FGL J0103.4+5336RX J0103.3+5337?ïþ_cè²±?Oµ˜y|?*	Ãwg3(?Oµ˜y|?ïíŽËÀ?hròq:?˜?bq4<Fþÿ?hròq:?˜?ïÌ÷ÁÜÉ?'qÕï"ˆ?yò"9ޏ—?'qÕï"ˆ?ïìބI5?K¨$Hó?c!{zr«z?K¨$Hó?ïþ'¸åöP?!zÑm–·¯?&Ôsgͨ[?!zÑm–·¯?濾"o€c?"èÃPáÀ?†^Û.n»:?"èÃPáÀ?ïÌF–8;?ƒ]«67/?yÜÀT€J<?ƒ]«67/?ï×£©×™?e6afNt÷?t.+åH?e6afNt÷AGN4FGL J0103.8+1321¿ÕîÄz)"ÀH³ïàÎ'À: ù™´qŒÀ<‡ú'+6@ùOH<¯´?þê»m(ø?ËBq¿ŠïÞ?»šÚ¡Ì˜õ?ðÖáù"»¼@³!€nÅ¿Ù"K"bа¿ÓŒIåQS¿à*;½ÆI¦¿ØrÁžEzÞ¿åSUèiáE¿âæqqAGNbll3FGL J0103.7+1323NVSS J010345+132346?ïÿwOÓãþ?‰kBT2?@¦'?‰kBT2?ïóº
œ9¡?[܎ÄÒû	?X‹äðÈ(?[܎ÄÒû	?ï÷™Ñ;¶(?bâR¦Y0I?PÌ]_X_z?bâR¦Y0I?ïþ{µÐSa?¸[Eõ¾?(D -è9z?¸[Eõ¾?ïÿ¤LÈR?í=ƒ	?ìÛ|/ā?í=ƒ	?ïËÙI?ƒH?zYl¹'?ƒH?ïû·ñ?ë?S¼R²¦š,?A ;"i=Ã?S¼R²¦š,?ïü©Þ$&ë?+V­çék?:±
Ífs?+V­çékAGN4FGL J0104.8-2416?秮%¨í0ÀUv<òϕÕÀ9î
^u×À<|ŒbyqÜ@HÇ nM@>Vð†?·‰áÚiÝ?º!²¾iîÂ?ûúÊ8Ö@ Î|O[Þ?æÇ¢u‹G¿ã¬ ‡t~¿èÉ—ïun¿é£J‡ãŽ°¿äæZb!2U¿ïÿÕ7ÕYcAGNfsrq3FGL J0105.1-2415PKS 0102-245?ïÿLW'¯?äƯq?6l¤Ÿ+\?äƯq?ïòêÓ?z?dšo—¼nŒ?Z*YšK?dšo—¼nŒ?ïò;_ÀY?EÍý08HC?[‰A8¾M?EÍý08HC?ïþäþP?Gû<±:?!¿oR"V?Gû<±:?ïÿ©¢•£?ãþ"?—U®Kä²?ãþ"?ïÌ®±{/?†-ÉBÂ?y¨§TFl	?†-ÉBÂ?ïéƒ1"aÕ?i›14"É?f|Îä}cE?i›14"É?ïüýXÓ"I?,ì%dpƒ
?89ܓŒ+?,ì%dpƒ
AGN4FGL J0105.1+3929?!t€À7Lq²•êÀ9åق½µÀ<m›2öÍ@ó	WA°O@ß^Ö?¶2«M÷?´ëÿ—û3è?üÅ,ÅZé@‹&NÉ;É?éRøàÑçi¿æÈ8–¿ã:âŠú¿âŒ™ÖÖ;¿ìæÍߜ]C¿ÜC!þ,–6AGNbll3FGL J0105.3+3928GB6 J0105+3928?ïýCÈ+ÓC?*Þ֔õki?5á½ ÆÁ?*Þ֔õki?ïõrB'¡®?XV	°°ù?Uz…ó?XV	°°ù?·…›i?‡Ì·6	<Å?‡",W•Ì?‡Ì·6	<Å?ïüÃb?æ?&»ò3·†?9äïv¤…ß?&»ò3·†?ïüãk,Á?/¬#ˁώ?8ãhˆ?/¬#ˁώ?ïÔ%‡+¶p?€€­ß&¹¤?uí<'ü?€€­ß&¹¤?ïÊ'Û³'à?'HtAïÜ?zìITB?'HtAïÜ?ïùÝQ:–?:kŸ»"
?K€Š/rSú?:kŸ»"
AGN4FGL J0106.9-4832?éà:ÓÄwÀQsWæpãÀ;råx+‹À<îã>ÿP@+Ç¸æ¼@±¦»ÁÎ?ÉW_ã?ó¿³ÍØ®?ã,Àþ7~@¼È}‡À(¿ë­AJÅ¿èpúß.Ï ¿Úò yI¿àIÏâ€é¿ïÿ¶.$Öy?ïü¯ž=Ã/AGNbcuPMN J0106-4831?ïôTBCé±?ZLÖ/gšÆ?WW{±æ
Y?ZLÖ/gšÆ?ïõnLõã-?W­°¯‰?U#f	:æ'?W­°¯‰?ïV3— ßÎ?íËþyK?•9
›ÔD?íËþyK?ïýÝP}›â?!7/)(çW?1|—îW?!7/)(çW?ïìcœ÷5ñ?fÓ÷†ÝEë?cœc3e7?fÓ÷†ÝEë?ïÏÅy‹ ?'rb^t—?xC4ð'?'rb^t—?ï˜:	ç
?Š[³þ÷K¹?‰ûñs7i«?Š[³þ÷K¹?ïë-?J»?`žëÂζ?dÒÀ—iŒ?`žëÂζAGN4FGL J0107.3-1210?ëM2éqÎÀR¦JŒL˜À:ºœiànÀ<ŽO'…€@ãg_ƒH@8>ž¡?ß­¯Ñƒ?¶ÊÿB?ë}?ó>~:˜'B@F
ú"†4?×·IbŸ‡o¿ß@zC'ý¿ç*
Osۚ¿á}¸èi¿ëÆÏ\Ê¿º¥@v'AGNbcu3FGL J0107.0-1208PMN J0107-1211?ïýŸl[6Ì?,/Ö¢¨Ë?3žsp‰a?,/Ö¢¨Ë?ïï$¢:–Ä?hñ"¿–?`Û]‹¯Ì»?hñ"¿–?ïáÌë¢ó?tͽú_@?n~3S•Ü|?tͽú_@?ïù@tÔ8?1ºšA?Jþ-ˆSæ?1ºšA?ïúETâŸ6?C/• ³«î?Fê¬f«?)?C/• ³«î?ïÄW^qá€?…J#¿Á¯4?}ÔPůh?…J#¿Á¯4?ïÖËLÞĶ?€[ õ¯?tšYÝõ#?€[ õ¯?ïßéœÁ?]çf'
¢`?pw^´¿…?]çf'
¢`AGN4FGL J0107.4+0334?Ô<Ôÿm«LÀM‡æÕw–À:ˇõ,ggÀ<_"žy_@½$x°?ù@chºÔ|Ä?Äs¨è茿¬/ñ¤|O?â³Jå×_Î@Rú_W(†?ï–ÄÓG³¿â^•ýWÚ¿äæAGÈìm¿äpý÷<7¿Ös©Ïr¿ïÿò> wAGNbllPMN J0107+0333?ïþðG?'?"mÓqî? ûFiÕ ?"mÓqî?ïòã›V™P?`¦"8´Q?Z8ÈßZ€™?`¦"8´Q?ïõ…5"e?Scb`×`?UõÊ5Î?Scb`×`?ïÿ+ÆϪ?J':é',?‡#¹[×?J':é',?ïþÔLæŽ?·EÇ8íX?"¿ÊFK®?·EÇ8íX?ïÐsÚ\N?|cÔ¨@?wÆî%?|cÔ¨@?ïòˆ3H_s?f>"Òšî	?Zï™2Çú"?f>"Òšî	?ïüƒXåtc?2Ðn|¬´§?;å7D#ÿÌ?2Ðn|¬´§AGN4FGL J0108.1-0039?î՝þz'8ÀO_ïIÏÀ:;+@ªÀÀ<}7%@'/m@§'…€Þ?Ä °¤£
?·p²o©[.?ñƒSV¿)v@Ph$»¿àd¤à¹)¿å[ÃÀ^ªZ¿è{.¿±q¿å¥ŠžT~¿ïÿªoª²Ç?¢''%ߍšAGNfsrq3FGL J0108.5-0035PKS 0105-008?ï÷"(«Ç?IçY¶?PÙ®jµ£4?IçY¶?ïî_V|¹d?aÖÖRgïé?a ©\Êü&?aÖÖRgïé?ïǕP'GH?yÜаD?|5WÑ©O¢?yÜаD?ïåöúü=±?S/¸Q'â?j	øÎË?S/¸Q'â?ïóWT?b,ºÓc€?YÚáÏɚ~?b,ºÓc€?念ÒÏèƒ?`ÎÚgA?†W]3ëH?`ÎÚgA?ïžmÎå€Î?ˆ‰¸·'ZH?ˆdŒ5qÀ¦?ˆ‰¸·'ZH?îîY§:ä?'º'0ÆPÅ?¡ox ·?'º'0ÆPÅAGN4FGL J0108.6+0134?ïÔl+!kàÀN~ß?–À6ÉÁö¯õ&À;)׆d2¯@ìPGk#@FtÃ÷;5?†j½ýÀÏW?º²ËCàª@-ùmL3µ9@!‰q S²…¿ËÅaž€‰¿áÆ,¿Ñ'®¿åû"y™¿æPÕÛiH¿êk¹AT´¿î¤;I'*AGNfsrq3FGL J0108.7+01344C +01.02?ïÜ:k5Ù?'¿žU1?qâÊX´è!?'¿žU1?î¡¥ƒK"@?´9¤vÎZÅ?¥å§Î¶gù?´9¤vÎZÅ?îú‰©6šœ?š$\t­Îp? Wei&ºH?š$\t­Îp?ïÀ)ÙBQ?‹¹AïRx?ëD
‡ø?‹¹AïRx?ïß"6$™?gÁu´?À¾?pnå¡;·?gÁu´?À¾?离øáu?ӞÝ7 w§?вˆ=Æ?ӞÝ7 w§?ïx«öœº?düâqØ=?ê,(Ä?düâqØ=?ë¼U_?»Â¡‡œ
Š?Áú«Ïž†?»Â¡‡œ
ŠAGN4FGL J0109.1+1815¿ïý"#–]ÀF3¬ÿiÀ9'Úa
À<8.j€@q©(ؼ@cH¿Œrj?²µ÷‹'?¯Èî_³]ª?û'{Gžû@?Ï y¿ÜÜCB	[¿á®†ü#»¿ÜÎÊ}è
E¿áäÃßt¢¿á>yî§z¿ìþ3!?•ÂAGNbll3FGL J0109.1+1816MG1 J010908+1816?ïù4o{ìh??‹àáÏËd?K.BÑÑ÷ô??‹àáÏËd?ïí"è)?coÁð*?b{ýe"‰?coÁð*?ï»SÊqA¦?'¬á¤
#Ÿ?+
Y¸¸®?'¬á¤
#Ÿ?ï¿^䀷d?g§by•˜?€(Fë(ÜÞ?g§by•˜?ïé
b&H?]€ØrnŠ?fõêv×Ô?]€ØrnŠ?ï¹a?àë"?"ƒ±™ÎD]?§°{©A?"ƒ±™ÎD]?]âs?Š±þ6ɍ?‰•h"G4?Š±þ6ɍ?îàJýn'?A:?¡ûP,Ž	‹?A:AGN4FGL J0109.3+2401¿é©ZõÍ®ÀCUGNΚÀ;¼|óp¦À<xwiÃèø@X.8¢ˆÖ@ç¹Å‰­?Ǭ0,–¿Ÿ"|Ái
Ø?ÕZ@ÿÚÁ@‹›˜w?Û¯ç#e4ã?ãeC»¿ê$kºc=½¿Ê[ê·nkÿâ["ötf¿ïÃ;ã?ÖAGNbcuGB6 J0109+2400?ïþêw
V#?š`TÒ?!X'ìÛí?š`TÒ?ïô&Z)8«?Z•¡ö=i?W³K¸j)?Z•¡ö=i?ïó>žÿ½™?VÃÌ6éë?Y'ÁÁKÿN?VÃÌ6éë?ïýh¿˜B?¥ÐæFn?4º¬üj3?¥ÐæFn?ïýž¯ê$2?49´qêÃ?3
¹·'?49´qêÃ?ï× X˜¦?u5þé?toÓª¾k?u5þé?ïò£¦bÕ¸?f:"•ñ³Õ?Z¸³M'_Š?f:"•ñ³Õ?ïõ˜œÞ6p?F¿âýµ ø?TÎÅü?‡?F¿âýµ øAGN4FGL J0109.7+6133?ëJwçݟ¿ó¸SH|p"À8-Ðé'ÿqÀ;áÝÖ	Œ@"ÑéÂ&@""ãw3=?¥,È
`)?Ä=2»i"-@–6mzVÞ@hZm߬x¿ºÅM~¸î¿áœ§ê9¿ç΀2ÀG¿éokþUÛÕ¿í²˝!ä¿ïÿŲýîAGNfsrq3FGL J0109.8+6132TXS 0106+612?ïÙè—rg?vøhbÀ~?spÆ$Ĉ?vøhbÀ~?ïԕܩA`?ƒ54KShò?uµÍ{Ô?ƒ54KShò?î#1ïwƒ?¡à|V7¦'?¯
Ìãœ<Ï?¡à|V7¦'?ïùîÆAž?;õñ™T?HDèúe¡?;õñ™T?ï£[Wr5Z?…†C^K%H?‡)*D‹?…†C^K%H?îˌÛÆ?¼£ÅA"?®G6"?¼£ÅA"?ì¥HBE|?«½&ÆÑ%Æ?ºÕ½ïÔ"?«½&ÆÑ%Æ?ï×ße&d?jퟖI9?tv<>Áÿ?jퟖI9AGN4FGL J0110.0-4019?×5÷UXïÀS™Ì¢ÛÀ:õ"£Ö3À<­9©nù³@ ›èÔ?]?û!³Éƈ?Æ	E£ù?ÀüÆ$<k?ú÷YhQ"@¹ˆºa¿ïÿ¬=`2Æ?ïí«3õÐÒ¿Àµm ‹]¿ÜϞƒŽ?s¿èU²Ÿ$?ÑÝсèMAGNbll3FGL J0109.9-4020RBS 0158?ïÿƒ™Z¸?òȝÎ+?ªçýÓ?òȝÎ+?ïö$"¡÷¦?V¾¨;n?S¶Ù@³˜?V¾¨;n?ïí"Šo?e¸½ÏÈ?bäÝ8™2?e¸½ÏÈ?ïûøP€˜c?.,û'†JŸ?@¾‡ҁ?.,û'†JŸ?ïý áR–?8­A͑!U?6øõ¥)3ò?8­A͑!U?ïÒ-?š!øþL?vñ÷ö9ŒM?š!øþL?ïÒ×r'?|\åp?v"FóSO+?|\åp?ïôOۙU?OÎò‹UZß?WaıAvX?OÎò‹UZßAGN4FGL J0110.1+6805?áàÀ­Ù©@(X¡ÅgÀ8qö_mMáÀ;¥Ý·Ö›ƒ@ %jvÁRp?ÿʘû(¸?¢6ÿ#>Ò?¶n]øû÷?à¡s†Ž$@qÓ%V{¸?ïßÑ÷®ø¦¿ßA–bØg`¿âýÝÄ쯿ݤÙÿj+¿Þ…"/_i¿ÞJ™¡|<AGNbll3FGL J0110.2+68064C +67.04?ïûº@G?6pӏ`f?CŸ©šc&b?6pӏ`f?ïéJ5ГÎ?m£†z?fµÊ[g1£?m£†z?ï}>3TÂ?'€ãyB©?X9š-ýº?'€ãyB©?ïˆ
žï?€£[•w(?ýzQ›LN?€£[•w(?ïíĜ…:?XKÊ1PªÉ?bñ;U¼V$?XKÊ1PªÉ?ïZöFÔáÕ?¢‡[Ÿj?"¡7,BýK?¢‡[Ÿj?ï\yǟÅ?"bòô±þ?"}0Ì3q]?"bòô±þ?ïÙP¾´?'åÑÝV'—?ŸÝ"ÐÀ¿|?'åÑÝV'—AGN4FGL J0110.2+4151?àöôAl<À4à@žUÀýÀ;¦ºq€uÜÀ<Ðà`'ˆ@"±ñ°Ü×1?úH­ž3\N?˚R¼iš?'òk—Ó›É?ʉ8x[@¦èxyä¿ïÈ8}õÏ%?ès5Â¿æi
_¹ùá¿ÅJâ&{>æ¿Ï&ż9¿Ò;lˆÌÃAGNbll6C B010709.9+413321?ïÿ'uÕ^?(²ùˆ?bšÖ"[Ì?(²ùˆ?ïõöþ4ßí?\põU>
Q?T2eÁ?\põU>
Q?ïòIùÉ/3?jçyzƒ?[l²Yȸ?jçyzƒ?ïþÚ~Ä´®?¤–Žvx?"X옮8?¤–Žvx?ïÿ»–2u¸>û,˜K¨?zsíC>û,˜K¨?ï×\$e‡f?{%@lâ?tQí¹N'C?{%@lâ?ïóñ4?r=ÊmÑY™?Yàx¦ù?r=ÊmÑY™?ïüųå?8È©ç'¶??ùÐû€uy?8È©ç'¶AGN4FGL J0110.7-1254¿ï—~à–êNÀRÄéÌ·ÔÀ:¾šþ§±À<Š®ª¢ÖY@½iLʳî@Pys‡?¼p1v´½¿–û^c@J?ÞÔâÛVþ?@9ä>-,?ïÿQ÷GË?ãÙª*áU¿æp·'¨å¿ê\Ïä¯B?µ¦ï|¥¿´Af|¶´ÝAGNbll3FGL J0110.9-12541RXS J011050.0-125455?ïý"Öq™Ô?0VCj‰Úp?3ÙKÓÂ?0VCj‰Úp?ïïÊã5z?hM…ÊÿË?`5¹«?hM…ÊÿË?ïÔÖna1ž?u0³|¯¬?u"ÈË÷"ë?u0³|¯¬?ïû}Ÿh´?2[^ˊ¡2?B	Ñêë?2[^ˊ¡2?ïú.—dƒ?BÄ¥ê"Q?GŸEW©©?BÄ¥ê"Q?ï¸CˆuÒ?ŽVÀ¹À–ä?ïóóª?ŽVÀ¹À–ä?ï½Ëƒ_¤?ƒþRݛǴ?€>(Æþñ?ƒþRݛǴ?ïé+Ò³Þ?am-$ÝLO?fÔ-âŽòv?am-$ÝLOAGN4FGL J0110.9+4344?ᵊ<À2ûÕýÍö˜À:Þc'í"ÓÀ<Šj}L[ù@"'ÌñŠÇ@á߃ˆ¶?Á1¨r¥d?vëþà(è?½ªñ°±ä@Uuów0Ž¿'…ÅYïh6?ת#Õr8¿éâ6Ó¿é ž9$å?Å~{
ã3¿èŠ= ÿ:AGNbcuGB6 J0110+4345?ïé¼_þS"?žo(|¬ì
?fCŸïÎtb?žo(|¬ì
?ï÷'ßö}Ô?R	ÈSoì?Q°@4˜@?R	ÈSoì?ïç§ÞÎ#†?nüV"qk_?hX!ŸéÆ?nüV"qk_?ïÿTdíP·?€.«a?s[ǝ¶»?€.«a?ïùˆ:²¿—?N.ÎÂ?ò?IßNŠÝ?N.ÎÂ?ò?ï×eka?'°ÔÅ?tvM4tO€?'°ÔÅ?ï̂Ýóï.?€¾ø¢`a?y¾ð
é
?€¾ø¢`a?ïüËãÌKP?2àFž¨éR?9 ã&,"?2àFž¨éRAGN4FGL J0111.4+0534?ïºB_岑ÀLxYÈÉ2À;r.´ƒ*À<À±Ù+€@ Øp±?ýñ´âg?Òص8[' ?Á8CyT?í6ͼ¶Õ@p]i!­¿îù/Lñ ?ïý°šgó¿èÆvÁþ<±?±e'«é¨P¿é.&ïX¿Ìò¦%C1AGNbll3FGL J0111.5+05351RXS J011130.5+053612?ïþ·ð5¡f? =ÇZ'DE?$€øÙñ¹(? =ÇZ'DE?ïòmjç?`ž'Qä]g?[%*e;?`ž'Qä]g?ïÛpuwÀ?t§'[—‹?rGÅ'C;@?t§'[—‹?ïûIIÊú:?/™"MM»%?BÚ×ùÖPŒ?/™"MM»%?ïþpªÉ(?,nÁÚÐx'?.Xøæ8­a?,nÁÚÐx'?ïÈ(%Vž?÷¯-k!?{ëðŽPðÈ?÷¯-k!?ﵜq1½à?ˆ7¤I/zÀ?'˜ã¯Èö ?ˆ7¤I/zÀ?ïíݤ>î?Z3\üj×2?b"[»
Ú.?Z3\üj×2AGN4FGL J0111.5-2546¿ë­Û`ÀUR¾7ޓŸÀ;0÷b¢Œ‡À<¶53¾sn@C¤Ýšzj@'Ýãu†?ڊVwÜ?È žE¥Ñ‹?íÓõƒ¥@	Óf'Ò,¿í!*¢jùs¿àÈ3?Èlì¿ä^1¾éà.¿áp—AЄè¿ïü楻æË¿ïdÑ`…PâAGNbcuNVSS J011130-254531?ïüêBÃ7ç?1	ÓI…Þe?8­éÎQ¸?1	ÓI…Þe?ïóM#8-2?cÁZ%×/?Ye¹ó¬ÿ?cÁZ%×/?ïÅÖ®¢ë'?x!²Ž§]?}¨ð«?x!²Ž§]?ïþxñ¿‡?ÕkwŠ`?/¸r-âð?ÕkwŠ`?ïþ™/ˆÑ?"¤Öq©8€?&mèï1&?"¤Öq©8€?ïÏo0†Òå?ù.ë&?xHg£)q³?ù.ë&?ï—éƒfÒ?†2¢ ›™ä?Š>˜Gx?†2¢ ›™ä?ïù ÜÙà?BL˜Ø-ü¹?KÁ|‰ØÏA?BL˜Ø-ü¹AGN4FGL J0112.0-6634¿Óƒ·*à9¢ÀI6<tûT À:S@FA,ñÀ<•Ór²@ߟ²ãA®@gFÂú?¼˜ðý-½¨?¾
iõçù#?ýŸ¼ÉIŠŽ@	š"‡0áI?ϓ˜8E–¸¿è÷̊‡­ß¿æf'Ï ¼¤¿ìj`%څ¿åÁ/ÀbY¿ïöm_~ë˜AGNfsrqPKS 0110-668?ïÿ#ª1ÊÜ?Sb…e`?ŠµéÏ?Sb…e`?ïö0§$G?T¡N÷¥º?SŸúÍ4Rw?T¡N÷¥º?ïðr€óR?NÚç{æ8?_ãSO«·?NÚç{æ8?ïù:âæ$ô?68¯ó7?Kt2§Â?68¯ó7?ïþvÊPŠv?-4¾	Œ?("W÷ã?-4¾	Œ?ïÔ:åî?yæ¯ÕÐÁ?uùâs9?yæ¯ÕÐÁ?ïÚSÄ´`«?wCŸãæs?rÖ¿ì² ?wCŸãæs?ïÒWªz¬2?hV}bà_?vÔ*¿ê6Ð?hV}bà_AGN4FGL J0112.1+2245¿î$¡
¸PûÀCïmÁ¤zžÀ7MØYÈÉ2À;%IfË@'P¹+@¼Ú'.?'/,¾O¢?­:­a2Ü@.&,ƒí@2od;黿"ZUû£é˜¿ÝŸâˆö´'¿á›žV—¼J¿á1xþ™x¿ãò«G£¿çåøL­W¼AGNBLL3FGL J0112.1+2245S2 0109+22?ïùL_ݔ?Zü'
ê.?KšÍþ>çç?Zü'
ê.?ïêΫ|ΐ?jú¿à·…?e1TEXx?jú¿à·…?ï¾ì åÂ?†m!uÙf‡?€D×æ%wU?†m!uÙf‡?ïø$"ՁÊ?>µIŽ²ÚÕ?Om¯òçDU?>µIŽ²ÚÕ?ïú¿(ÊN˜?Dfq:¡?E]¸+ýÍ?Dfq:¡?﫲ãízÂ?–Íï:°?…Gð#b?–Íï:°?ï݃6çÙÕ?wL/^?q>d¦à	"?wL/^?ïæx i†?\j7d?iã‡M¸Ô?\j7dAGN4FGL J0112.1-0321¿ìK¤2œ+èÀPnk΅3±À:MÞÌ©'^À<YÙAOU©@sLYŸÙz@Öðd‰Ø?ÁË©â,£?ÂÞt"ýS?ýJð
­@IV‹'?훀#¦Î6¿æþ*¿æèɂ•q¿ê¯ ²¿â¦=Kºéu¿ïÿT©¥€XAGNfsrqTXS 0110-037?ïþg÷,"*?!Ji…?)€ŒÓȟƒ?!Ji…?ïðc÷ž?`Ö·Ò׸??_9âÈô??`Ö·Ò׸??ïïbÎ×>?MtoÁ¨?`1Ã+,?MtoÁ¨?ïñ­Ï±ƒ›?Cg÷UwƒØ?\¤`†ûIÉ?Cg÷UwƒØ?ïýºÂ´?4‰äÙ¼6ž?7j+
q ˆ?4‰äÙ¼6ž?ïÅ_0Î:F?Ý¬«©?}PgšB´Ï?Ý¬«©?ïÓٍ¿5?tñ¬^"	<?vS=mŠ?tñ¬^"	<?ﬓ!c»?qúV؇˦?"Û7±¥F?qúV؇˦AGN4FGL J0112.6-3158¿ïÂõù@ôÀTÓü;OagÀ;®¬A<
rÀ<õË^7ü@ m®@o±¿?ö
þ`Ï?ß]àÛÍq?ç\3rSÎ@"ìck	c@ÃüÏHýö?ê³rôb³¿ïÝHæ"ß(?ìM¤=Œ}|?¹–@bŠ~¿áÒ¨ëÎE¿ïùêqùA AGNbllRX J011232.8-320140?ïù#¬Ïά?CÕ=ἆ?KqMFéAo?CÕ=ἆ?ïðܑeîq?cxæà»r?^FÝ9¢}4?cxæà»r?ï´Ò}ö?zÕB=Bz×?'Ë`´ËL8?zÕB=Bz×?ïãk"ÞK¥?[Ö1J?l"{QÎâx?[Ö1J?ïöwþ¿8:?QËs
Å6À?S¢‹Ìx?QËs
Å6À?ïÖ¦[ãš]?t‰½ '*?t¬Ò$0Q#?t‰½ '*?ï¬UX¢Ÿ?†;)÷Ræ?"ê©Ô¼U?†;)÷Ræ?ïÒ,äuÇ?s}¢É=S!?v鍹mʶ?s}¢É=S!AGN4FGL J0112.8-7506?ëûäû RyÀDù}¿HÌÀ:ZíÍÎTŒÀ<'йÁWN@»Þû£yí?üž_ ÷Ç?ÅöX¡×«£?Ëë4Áӟz@@ìYZi@Þ+"ƒZ=¿Ñðh}—ÛS¿ä¡ŸAÏ-O¿à¯¤Ùš¿Ø5X§ay¿áá»;ªÐú¿ïè ÓI¾AGNbll3FGL J0112.9-75062MASS J01123146-7506179?ïðâ‰U1h?TRiCÔ?^:íËϾ›?TRiCÔ?ïìÌJW"b?a[g3²¶?c3µqãÞf?a[g3²¶?ï½Rlš™/?{ý¯¾Ø$?€«dÏbÖE?{ý¯¾Ø$?ïȃ쫆Î?_‰¾Œ˜0?{¾	ÂIÜ°?_‰¾Œ˜0?ïØ2ŸB-«?p¶àè'Å?sæ°SêjÇ?p¶àè'Å?ï³uAêâ?…—"'5§?ƒ"¯Ï[]w?…—"'5§?îÞðÍvڗ?™è–ö´Ï@?¢ó%þ¡™?™è–ö´Ï@?îà"ä"ÿ´?Œ?r!S¹?¡öÁ¾«ë¹?Œ?r!S¹AGN4FGL J0112.8+3208¿ê^,dH:=À>ƒâCV—À83È23XóÀ;Äöƒ{á@Ü4d`§¶@<`Ÿ?u¾Ú,?±#™¸"pÃ@üm'ºZ@ÊwàŒGL¿Ö':ÛG¿áÿe:í;Ø¿åú#G,å¿å €sWæq¿êLÞÕãÌÄ¿åÄ|ÁNjAGNfsrq3FGL J0112.8+32074C +31.03?ïúè©w2<?:?ìâ1ª=?D]Z–4N?:?ìâ1ª=?ïòˆùÄ?aÁ?ÿ‹K?[üX÷?aÁ?ÿ‹K?ïÚÚєª?u#8áíI0?r'—~*¤?u#8áíI0?ïÿ¯P÷$ >øÜ*{)Ð?+¶M<êÊ>øÜ*{)Ð?ïý×
e?1bù¡?7II(†L>?1bù¡?ïÎÀÒe	'?y›íMu%?xŸ–È«ÃN?y›íMu%?ïáévü‹¬?z\¸=Ͼ?nˆç÷sà?z\¸=Ͼ?ïÿsØaLî?V"<::Ï?"õÅ)½?V"<::ÏAGN4FGL J0113.1-3553?ïþÝpˆÿÀTß«÷jÀ9Ûà$˜e½À<'4pJ@"{ZqÍ@¯ÎÄô'7?³îހº‹¾?¶ÞGH"íˆ@^á½Ùà@Sòt|(Å¿Ï<í[¸{¿àҟt¤í‹¿ãýDcÝ*¿é oA{P¿è?b`ÈAοïÿ4Þ®÷zAGNfsrq3FGL J0113.0-3554PMN J0113-3551?ïî®;''_?•ëë;›ä,?aQÄsXŽ?•ëë;›ä,?ïöºÆSЦ?SðŽÁ£÷µ?RŠsâ×?SðŽÁ£÷µ?ïê'/—ó&?m€¢(;¹ç?emЇ©A?m€¢(;¹ç?ïÿ±| u½>õåá֎Ç? Ø¢Qûø>õåá֎Ç?ïþØÑñW?+u¯'y?.Rp0Ÿ2Ž?+u¯'y?ïÝÏ÷N«Š?rÁJ\unè?qt×?rÁJ\unè?ïÂ{&UÃñ?'¢¥'éT¬?~Âlí+K?'¢¥'éT¬?ïÿ`d?¿zòòˆê?ýèW
Çæ?¿zòòˆêAGN4FGL J0113.4+4948?㓘p=kÀ)ÒŸ˜·À8Ùì©&¥À;ºÇply¦@˜ãy·|@^·E|?¦Ñ›¯ô?±™é¾·5@
jÊA¤æ@èæ5?íԗœiW²¿ÜÎQÝr¸¿ã^ö€$}Ž¿ã}FA­¿ãÕ4ûE†¿çä]­Z@¾AGNfsrq3FGL J0113.4+4948S4 0110+49?ïþ<œúˆX? Õ"Ž¶¹?,60`FKÒ? Õ"Ž¶¹?ïô‰ÑiXx?b,€Ui­²?Vì\·€¤?b,€Ui­²?ïë{l‰Á?f%[z>Pn?d"ïÂ0î¶?f%[z>Pn?ïÿŽKîÒ>ûo+;×4Þ?m"–0>ûo+;×4Þ?ïþ<%A¥^?"J6tâ¸Ö?,=®=ÿrT?"J6tâ¸Ö?ïôʙä?ˆžM£èK?~%šÓZL~?ˆžM£èK?ïÝ>ànò?v勋=#5?q`æ~*ÿ?v勋=#5?ïÿV§#t?	Éú…ìQ?+Ð\¬?	Éú…ìQAGN4FGL J0113.7+0225¿á¡îÆpàÀMûïÝëÙÀ:h†Úz4zÀ<rû@
faÞÂC@%iF·G?ÅbB¶3¿›y¥ÂÇ»?ÑÞ`þW@@}8ém¿æó0¿ŸÛ¿åNx¾­¥?¿çœÕÃìS{¿ãR&]·Á"¿äÜ¥‡äe¿ïÿù³>†AGNbllUGC 773?ïü~#؈~?0ːíB?<áÖÄö?0ːíB?ïñÃL?`jÕß¹š0?]Æyƒôö?`jÕß¹š0?ïî0ôOÚ?d×ig¬?aãÏ/†5?d×ig¬?ïûŽ`wÜR?(ã_Œ€?AÆ~Y.®N?(ã_Œ€?ïû݀›";?6í{Önà?@‰ýöN?6í{Önà?ïÃo;!>>?"µiN@[?~Hbv@â?"µiN@[?ïÝÚÉ ?tø§òNóÍ?qt'˜cé?tø§òNóÍ?ïÞĊDMH?c|êcÄ÷?pºÐì?c|êcÄ÷AGN4FGL J0114.0+6418?î¼®ž'a³?ø£~éÐÀ:&xèI*À;Ëe±Ím@ ëW+5ý@)³(é-?ÅË#ÕGD¸?·£3÷(k?ìOQâJãS@=Šzº0?—p4£ý?ß&Á°¹ò¿âàKd'`˜¿×c§úÛR÷¿ç•¶ë¹÷޿׋²ü;AGNbcuGB6 J0113+6416?ïýØüíD?(.÷A›ýá?18Ù7?(.÷A›ýá?ïæ""·‰?vcËË›?iÝݍ±¦M?vcËË›?ïíœ4Bk¤?há‰ü?bcËäûž?há‰ü?ïöù–s8?=,͹NÞ?SÜ
"ï&?=,͹NÞ?ïû˜G'™S?AþÛÐ#?Ažâ)Á?AþÛÐ#?ïƒî?¯ŸRLEV`?žMç4D?¯ŸRLEV`?ï°š"ôÍ?‹LÌLÏZ~?ƒûYPËîÚ?‹LÌLÏZ~?ïá?'"h?`²£x7¸?nâÀŸW÷ ?`²£x7¸AGN4FGL J0114.8+1326?îr.¸*ÀH…S`Ð$pÀ9È=ñÓÀ<"HÏ|ª@%ôx7t6@ÔQ[<f¹?§JdR:	'?eŒQ1 áâ?¿ÝϾï"x@†ª(²ý¿ÜÀêm¬¿àùL`RP¿ão·]yØ´¿Ý×}_§/"¿ã:x øóò¿á5›WߺæAGNbll3FGL J0114.8+1326GB6 J0114+1325?ï¿G‹	M?±"lç†x?€.?©DN½?±"lç†x?ïõ,–¥¸%?Z`êì…Â?U¦Òg˜vù?Z`êì…Â?ïó©Ý€ñy?pL\Iãì?X¬EE"ì¯?pL\Iãì?ïþݕ
Øe?«M6‹¦&?"&«r·BÚ?«M6‹¦&?ïþ¥&ë|:?n³"—?%­"׋oÙ?n³"—?ïÓwï$æi?{"³ý²‡?vDŠiƒ-?{"³ý²‡?ïöaÕ¡Ì]?fIyKëmÑ?S<TÒdÆ9?fIyKëmÑ?ïþY‡äC?$]ýÂï?*g'©M]g?$]ýÂïAGN4FGL J0114.9-3400¿á^¥úrnÕÀT]§°³''À;_»QzÀ<¬zyBáý@!Á\+e‰?üÿéYËM?Á;–7¿ áŸlÂK?ßÚr\"Ô´@j¾—ÕÊ!¿Û2pžÎ¿èÕ?AßHz¿ß‰üÙ´¿â‡Ÿïôð¿Ëáw(Öc?|~Ó"Yú¦AGNbll1RXS J011501.3-340008?ïÿƒwˆŸ?"ÇáÑ45?"Ò?.?"ÇáÑ45?ïöM\)K©?Vî²/Õ?SeGú_íÿ?Vî²/Õ?ïø–yԂN?[çâäN'8?M¦¾tè³?[çâäN'8?ïÿ–Z
×H>úúã"0WV?
ioÉy}>úúã"0WV?ïÿ`q@^?_¬ª¨?ñԞ?Uì?_¬ª¨?ïÚ 2÷	s?sýˆ¢Ÿ&?r¯æ‰Jº¹?sýˆ¢Ÿ&?ïû½.I??^†-<?Cé%R	,?^†-<?ïþ<–‰Cá?'×71ÀÚ=?,6™iîSœ?'×71ÀÚ=AGN4FGL J0115.1+2622¿èwBbÙOÀB~|âÀ;Êön‡À<m|ßýa@8——¶Àq@MíHû?Ô3ÿ
z¿¬¨PÁŽ€6?åü·ÁLæã@
4rIs'r¿än?Ƕ¿²]¨@•5K¿é¿¥Ò.¿ÖKIàâi¿×*Â+A¿ðAGNbcu1RXS J011451.8+262337?ïÿ'Ò*/?ÿ¹NÓ?ͧ#]ðƒ?ÿ¹NÓ?ïõ˜-?Xl•^?UÇÓ ö)?Xl•^?ïîUvæ!™?b‡y	líi?aª‰·G?b‡y	líi?ïÿ3z3€i?+Ð#RšI?¼d¿9‡?+Ð#RšI?ïý êOZ?3¬âNDûæ?2ø°\?S?3¬âNDûæ?ïÙd§ÁÇØ?vKLÎrØ?sM¬/—÷?vKLÎrØ?ïç†~1»?sÁ(2E?hyY²}?sÁ(2E?ïûu·è?:²¬5ÿ?B+ó$ž?:²¬5ÿAGN4FGL J0115.1-0129¿Í¶:'BÕ_ÀOßbb˧3À:î¯÷ªÀ<7mƒ'˜@h€•'¢)@¶';‡?¾`¿øì?¹—´<25\?ò:e;Ãûm@6ƍ?îQB‰hI¿äµ€r'¿ë)ºy
2¿ìµÀÁ¦©¿ï'›??ï;-ÇüƒAGNfsrqPKS 0112-017?ïÿ	s:Š?øaóЖ¹?Þ"_€?øaóЖ¹?ïò¯B€áš?^ÂC
ށ³?Z¡{Ss°?^ÂC
ށ³?ïæv™¸?c˜ ›Ôý?i‰ä¿à?c˜ ›Ôý?ïýn®g¶?#o_ÀÇ^†?4Š‹Ú»˜?#o_ÀÇ^†?ïÿPÖŠ?ä]Ø|É?uãæ€{?ä]Ø|É?ïÍ¢|0?WzÓ?^Ž?y.ÁÌx?WzÓ?^Ž?ï݃JÅ™?u#dão×?q>Z´!ŸS?u#dão×?ïñè¯EAB?PŒÿ­¡Å¬?\.¡I'}8?PŒÿ­¡Å¬AGN4FGL J0115.6+0356¿ê¹¶éûJ¨ÀM0—á2µ_À8ûá÷|þÀ;ø­•Ïà~@a$H¸@Go*ZG?¬
é½ôAÜ?²"†Òeh@X>»&²@\ìj!¿äa³'¿Ù®=•ŒÄŸ¿á1QFC±0¿à†&˜ðý¿æüÁâc¿á1´âf'AGNbll3FGL J0115.7+0356PMN J0115+0356?ïþ4+‰NP?Ni—='•?,½IŽ©'K?Ni—='•?ïðV6Ã`'?`´Ž-í³?_S'hÀ»I?`´Ž-í³?ïî¶4Á?pa#ªØÇß?aIËvRE?pa#ªØÇß?ïϛï4UÈ?cëá¨bw?x2Oל?cëá¨bw?ïûHõÏ?<L;š 4?BÜ)šþøª?<L;š 4?ïÂ:ˆD»$?"6ãx¬*h?~â»è¡.+?"6ãx¬*h?ïËÔڍT½?'4cos"à?z'ÛÍn?'4cos"à?ïB´ì—~?‡æ4hA¦Ì?—©bdy&]?‡æ4hA¦ÌAGN4FGL J0115.8+2519¿à㳪M,ÀB›–À8¥´B'KÇÀ;¶Î¬ Ý[@Kn	È֞?þ¬*˅¤ð?£‹`-¸±?JïË
d?«*JX…@ãLÓi©¿Ô åΑ¿âyDÅ+áY—K
À¿ÛJÝÿz)¿Ù²†eà/¿Ý"o@ª•AGNbll3FGL J0115.8+2519RX J0115.7+2519?ïÿFT"A?öز1–9?5'¾ ©?öز1–9?ïöºd|?V;ûf¢¨?R‹7òƒÂL?V;ûf¢¨?ïö"áª?\ÑÒ¾Óã¶?R÷ҟ Ÿí?\ÑÒ¾Óã¶?ïÿóÂHÔ>ÑîõW>Ø{'
ÑX>ÑîõW?ïþǫШÏ?¡RWâ?#…FÐϐ©?¡RWâ?ïÔÙ×Tî¢?x
.Wó?u"7ü
õ?x
.Wó?ïöÚð?bu5¬E?SïУž?bu5¬E?ïÿù†¶>Ðŗ;Få>˟t)xÓå>Ðŗ;FåAGN4FGL J0116.0-1136?ïÿ£NײÀR\/ƒ{J#À9Aª>-À<?¯à,ûâ@gÈ;B¡@©½R†?©!="±l?­[Žœ•Ÿ@¢Z2{@Êæºßr?›­5F¢•…¿â"Üöæ{Ê¿æ·hí)c§¿ãY`>.8ø¿æ¿Zž\!¿ïÿZªÕ+AGNfsrq3FGL J0116.0-1134PKS 0113-118?ïþïRødD?Ôì¸ðK?!
ÎFȎÉ?Ôì¸ðK?ïò©(¾÷2?aCL‡¢^*?Z­®[,?aCL‡¢^*?ïë±Ökø?søý‹ë2ú?dN)É[?søý‹ë2ú?ïÿÊl?>ð@h0Šeó>úɹÚzÉ]>ð@h0Šeó?ïÿQɘ²5?•¡Æ΀?ÆÐÍxø?•¡Æ΀?ïÍeïYP?"ÁK…S­?yvÌôeœ*?"ÁK…S­?ïá©?vYñ?|cæ÷ËÊ?nVÀŸ£?|cæ÷ËÊ?ïÿ·n§äœ>ü 
½"•V?$F
‹7ž>ü 
½"•VAGN4FGL J0116.0-2745?àÊl9(ÀU ÃLŠÆÀ:ýayWÀ<Ÿ\>Å7­@!R'È>ô?ûšîcŠ	?͏t|©Ÿ?¾‰œKz§¼?ï
¾ßÏ3@" fQïýÁ̾Š?ïåt™/¿È"%Ú/5ù¿á½>!£¿¿Ø¥{úø.O¿ÔÁ*AÇöyAGNbll3FGL J0116.2-27441RXS J011555.6-274428?ïÿ¨Íû1J>úÿÅö¤™Ã?̍`"H>úÿÅö¤™Ã?ïõjOK?Z€ÚJ&b?U+aΖAq?Z€ÚJ&b?ïöàs6:?Aû	*š?R?ð:ëÜ?Aû	*š?ïýÒÝ̾#?F	˜:äú?1i$ÈlE?F	˜:äú?ïÿbTø™ž?²ïö]¸?µg9¼í?²ïö]¸?ïÖö.Î}/?võÂg€±-?t"誟`Ž?võÂg€±-?ïóㅲP?fuÜZ`(?X8ô%žÐ†?fuÜZ`(?ïúC×+†¨??0*CQ¨?Fð£ÐWz??0*CQ¨AGN4FGL J0116.2-6153¿êGyCbÖ9ÀK~r\=îxÀ:}ç&f¿À<š ]Øù+@ 3^(6Ö?üÈÈ@vÕ?»UÖ&"?´zڀƒaä?úcˆÕü÷?ýNá9–O¿ïó?']<?Ï\°¸¸Ä¿Î3BL«ª=¿áãyí+çå¿ÓQ‰_²¿âyUn"AGNbll3FGL J0116.3-6153SUMSS J011619-615343?ïýÁ`ÕOJ?$¼/‡úg?1ôûëIj?$¼/‡úg?ïòïÈ,?`E$5±?Z ý¤y¨(?`E$5±?ïë:\?iÏu¦†?dùü,;"?iÏu¦†?ïìc@žß?Lvº	‡{ ?cœ÷ždàü?Lvº	‡{ ?ïù%™Sá?FÕ¥×ÂKÆ?Ki›/ cm?FÕ¥×ÂKÆ?ïÀYl¶j=?‹—ä¤	(+?ÓI¯É¡<?‹—ä¤	(+?ïÞÍØTY?{í$W?pú
æ×q?{í$W?ï¤Bï¶(=?zIƒI¨—ó?†ïDU(¶?zIƒI¨—óAGN4FGL J0116.5-2812?ä"¬2sxÀUÎÙ‡+À;Zm]ÑloÀ<šVHáñ!@õ^*Ü#@ƒlØ?Æwe'+O¿¯]ÃT¨ù´?ãüµþT.U@ÆÞþ}Ÿ?åɛ?-±¿çbz¿å"u'ÊIe¿äê•ÀF+³¿Üãa¹®b¿á~ÁqN÷µAGNbll1RXS J011637.7-281146?ïþhe;q?#ο'ÓÚ?)y¯c͂?#ο'ÓÚ?ïõ7Hš?Y£ùô	?Uý'z¹'?Y£ùô	?ï÷+_¡ž?\Ã÷øßÏ-?Qó©•ó]?\Ã÷øßÏ-?ïþ¹ŸÚŒ?…@d.?$eþ*}_å?…@d.?ïþE:ØÕ?%sYøk5?/Û«dô?%sYøk5?ïÒe`ŠŒê?|áyƒÙÑ´?vÍO œƒ1?|áyƒÙÑ´?ï÷KÏÈeñ?[–kí/?Qh`ó%;?[–kí/?ï÷EK¹'Ý?G&f'ëÀ?QuhŒÜFè?G&f'ëÀAGN4FGL J0116.5-3046¿ï˜33øļÀTÙp÷¹àaÀ:üd^NiðÀ<¦ù)L)¤@»Ç{)@˜jßqë?Íåw©ïÏ?ÃD͏jk¯?ò\T)Md@ˆ|ñm@?ívѧR¿ã"Q´þ¿æ¾ç0ü!N¿ïþŸ½Êü=¿íjUéŸì?ì0…ÔÀ·AGNfsrqPKS 0113-310?î8µ9nr?ÍÄž÷õ?®¬t¬iâ?ÍÄž÷õ?ïé·'¸Ås?p®š`£Ï?fH؀óý?p®š`£Ï?ՙ'?…f£©ç[?‰Õʧw‹y?…f£©ç[?ïóÝ5-fô?D¬ž`S(þ?XE•`yèN?D¬ž`S(þ?ïþ%R}ƒí?.ÏgY+­!?-ª×YåØ?.ÏgY+­!?ïŸ-zY?"º²"dtm?ˆ94«¸'õ?"º²"dtm?ï66¦bÞO?'Fvôãs?™9+:ƒn?'Fvôãs?Dö]?›»~æü?Ž>+RÌÓ?›»~æüAGN4FGL J0117.5-2442¿í\ÏcÕèTÀT颣Y6À;ÁV¶JªÀ<ïCœ7Ì@!W"È×Ê­?ñøDIÛì?é!—c•?ބwžr{?ñ+k…L?ý;IÚ¿~±¿'¢Ïù'Ñ¿éôöí1Ç"¿ïí	þ±vZ?Ñh=¿çTbøóœD¿Öà¤E9¸AGNbll1RXS J011746.6-244329?ïú—nØ6?B¬-'ü?E¢D‹é¹]?B¬-'ü?ïðÇ@ø)?hªJìc"?^q€†M«?hªJìc"?ï§Ð¯c
?~öý G`K?†Ôíä"?~öý G`K?ïü#ë¨Á;?2ízif?>à¢úÕ-é?2ízif?ï÷Öhaò?Q%j¯bC?PSîÕæDü?Q%j¯bC?ïÆJÿ¥°?"æX9'?|ڀ"|è?"æX9'?ï›þíË
õ?ÿoÖ4|?‰DšúòÄ?ÿoÖ4|?ïôûãnW?V.zÕi?V8ÛÙ""?V.zÕiAGN4FGL J0117.8-2109?ïÞU¹®@ÀTa¯ž¾œˆÀ9lszKÀ;æK!JÓ@ÛBV¼¥7@¨¾e*ý?¶ú³åË z?½j°£vg@ý¾`l@½X~qJ?ïú"Àā¿×ÅÑZûú¿ås^ ò"Ü¿å锹`~¿æåªda¿ïú)âQ™PAGNfsrq3FGL J0117.8-2113PKS 0115-214?ïþy²ô^Œ?Ec¶"Ôs?(dΏïÚ$?Ec¶"Ôs?ïó@"æHÁ?`\¹püÐÌ?Y~؀e½2?`\¹püÐÌ?ïè5;B™?a}mc­A?gûÊÙ[@?a}mc­A?ïý«¢Í? îÙÀ¼ÐV?2¢ðéý? îÙÀ¼ÐV?ïþQ9â›?#=3í?*ìaÒ´žZ?#=3í?ïЎ¯Ÿ".?~ER$þý£?w¸¨ðU?~ER$þý£?マ z?€xtƒ$*3?€\ë¡?€xtƒ$*3?ïùÅæЕ?;‹/(&n?HëñpxÓ(?;‹/(&nAGN4FGL J0118.7-0848?ä¿B0ã3ÀQ¤Åm\ú­À:nÀ<~lê&3@MùÛùz@ÐÛä—Å?Ï1æÂlK®?Ò\'þw•@ùCM\ª@	Q¬«5x¿©È&ÊÅ
·¿æô¼U…ÿåë澚¨¿íb(E¿ïÿÙi"A'¿ã.<=óÖ|AGNbcuAT20G J011844-085058?ïý­$Ù?+"Ÿ£`C?2–Ù†
V'?+"Ÿ£`C?ïï2‰®Ù·?aAuÔ#'?`ÍvHç9‡?aAuÔ#'?ï¼j˜^?uÖ&k8X?€ÿe"øÐq?uÖ&k8X?ïì¹=g®T?J΁û"Ó?cF'ÒL3?J΁û"Ó?ïþ³Ph¼ò?'Aq;$\Z?$Êû`ů­?'Aq;$\Z?ï¶îˆM/Í?‹úNDJw?'D]ó"D?‹úNDJw?϶·?"Ï"R‹R?‰Lâ¡?"Ï"R‹R?ïTº"©‰?ƒè´oôX?•h­ŽO*ä?ƒè´oôXAGN4FGL J0118.9-2141¿êckWÀTnð¹À89¼R+EÿÀ;ƒ|@Ã@æ-Lê@œIwB?‡B÷Bä?·dD"@;p@Ú»£@P;\Í`q¿Äy
t­¿â<i"‰G¿äÄFwÜ¿â¡fµN+¿è6;ÏÆ|¿èéQ'©"AGNfsrq3FGL J0118.8-2142PKS 0116-219?ïû»Ì·?>ܦ£'c?AÐìÔL?>ܦ£'c?ï臓æ.ü?rÀ´úæG?gxlI닞?rÀ´úæG?ïÂÐ?{ž?"YHA÷j?~—à5"4R?"YHA÷j?ïêÔþ°°É?SÞ~$?e+yê_)?SÞ~$?ïìñ8£Þ?cÅ«);É?cǏ¿YÖ?cÅ«);É?ï«WÊùt?'-«›
C?…*:ÂòÏ?'-«›
C?ï¼Ù4ud?‡tL±s$ò?€ÿI®Ã?‡tL±s$ò?ïUSf"nd?‡"tI?•U"4™r?‡"tIAGN4FGL J0119.0-1458?Ç'(è¶bÀS†YJôñÀ:I£–ržÀ<V>Eµì¶@ {ßaúÆÛ?úgJ&"¿??Úl'p‡R?¾ÀRëà8d?þ1Ó·¢™@ÛEPl)?ï÷Ÿnc‹¿å2GzèÔj¿Ý¾6|=é¿Ñߢ'fŸ¿Û¬ß\‰É¿âÊÕFEAGNbll3FGL J0118.9-14571RXS J011905.4-145906?ïþ÷ÕAÄ?$Élµçeã?/ð¸®?$Élµçeã?ïòbŸ¡4\?["	Ó*™c?[:ÀÙ'?["	Ó*™c?ïêTÓÓ"?vØM†?e«+ñÚ%5?vØM†?ïóÝð(q??'"ªÛ?XD «^t??'"ªÛ?ïúš¦gæ?D	gD°¿?E•gµÂ
?D	gD°¿?ïÂð¼&r—?‰ºƒ-?~‡¢d\‹?‰ºƒ-?ïáu·xbù?€G=4ø‡÷?nŠHœ:®‰?€G=4ø‡÷?ïÞvšˆyX?]Ú韆7¦?pIJºc{î?]Ú韆7¦AGN4FGL J0119.4-5354?ŽM·Ý–7ÀO[ñ•1äÀ:ÙܲÀ<µm¿öûu@×o'yÇ@Â/BêÊ?À‡‰v¶Àœ¿¨§q@˜y?è[x¦@Y
\J?ÄB§Yö–u¿éqmŒ¿äüÅd"¿¿ßD˜¶DË¿ïóO]`XZ?âM‡rO¨µAGNbcuPKS 0117-542?ïú!€ûŠr?=[ݹÛ?Gyü_Z5
?=[ݹÛ?ïôD*ÚÒ¨?Xå|rÉw?Ww©Ô(!Ž?Xå|rÉw?ï՜œP{?iڏ$ïý??u1óªHžÃ?iڏ$ïý??ïù;Ð?8g]u97?KøââÖw?8g]u97?ïí°‰Âƒj?aGã5pW‡?bOv
b?aGã5pW‡?ïÏNïs¸+?'à²CqâK?xXˆI"†€?'à²CqâK?ïÔPµá4?z#\'E?uפò‰9?z#\'E?ïË
-¼Œõ?mçèŽùZ?zzékñ²?mçèŽùZAGN4FGL J0119.6+4158¿îÑNµ«ÚÀ4"ó#x«
À;DÛ;$™<À<¥ˆI=‹@¾½º`8¥@Ÿ°ºG?Ð'L†@?È¿ˆ–'ýC?û®oÜV?þC,»–ï?ï= "Ds¿¯´Ê!¡»Q¿é6†…ÀŸ¿Ü»õy"@"¿í5Á¸œ" ¿ïÿX¥³ƒPAGNbll2MASX J01200274+4200139?輪ëÕ¸?™Wèõ!­?†?š
'?™Wèõ!­?ïŠu£´êG?"ÜsUY›?b—#óz6?"ÜsUY›?ïyd'5X8?"¦
‡j?ÓmÛÇ?"¦
‡j?ï°áߦ?}lçù"?ŸéüE{ÙA?}lçù"?îÀã;ú?¨HèØUW?£þ±ÎÔé?¨HèØUW?íŠNŠ–`?¹"ü#9†ƒ?³¯U‰ó?¹"ü#9†ƒ?îN(û?›˜7N2Ùj?«¾ ßêÿ?›˜7N2Ùj?èÙ 
Þ¨?°ª¾½¼û?̙ԇ½_?°ª¾½¼ûAGN4FGL J0119.9+4053¿ïëá©Ó¤À5¨¡œZÀ;œqÀ6¼UÀ<ØÐÜüŹ@ ÄLˊ­?þº"Àõ(6?Ø:ú݁O÷?мXáB¥—?ú*…ʯ¼@`ô)2(q?íÜã›EkD¿±uWELå¿Ûç};?¿Òuác\ƪ¿åÙþí[c¿ïô ~$É
AGNbcuCRATES J012018+405314?ïùMýË®?Bñ`?JÈ	žD«œ?Bñ`?ïëÑ	ûßè?bN[Bóz?d.õǦ÷î?bN[Bóz?ïÓßÞwo"?p
~g"ÜÂ?v®Jîø?p
~g"ÜÂ?ᅰ·ëFé?`ï…'rg?€'œ¡­?`ï…'rg?ïøt²ü¹q?JH$d»Ù?N-3NÓL?JH$d»Ù?ï¥A/»?‹™ocvX2?†¾o´:Q,?‹™ocvX2?ï¯YdÞ?"/^¬y–R?")¼wÏS?"/^¬y–R?îيˆ.¸$?ŽY¡»Ž?¢gWy¤áÀ?ŽY¡»ŽAGN4FGL J0120.4-2701?ïý(‰…-ÀT⹩çÀ8dµ—&À;YАä¿@øŠë«à?ý#8ê,Y?âWùf2å?ª²³_ؤ@ñ¡˜kœ@§é2Þúw?ïýŽ5¸H±¿ÙCSy¿Þ@áDž»¿ÚtZe&Jm¿âXQ€%TM¿Ü˜‹<3·èAGNbll3FGL J0120.4-2700PKS 0118-272?ïýQÃ}Sú?1¦¹‡Ä´?5qåKp"i?1¦¹‡Ä´?ïì"`û?kò"—8§ ?c{Ÿ°r*?kò"—8§ ?ïÏßnî}Õ?{îŠ`,m?xHž¾•Q?{îŠ`,m?ïÞ/'ƒ)?\Ìâ@ÜO?pè?,ÇU?\Ìâ@ÜO?ïú9€§k?F"M7w?G½Ilª?F"M7w?ïÄ~…I´?…OsfÇ7Ì?}À½nc̊?…OsfÇ7Ì?ï·{[¸Yñ?†»H¡V\?'!)("Ô?†»H¡V\?ï"qÖÔZ?}"Pâ9©A?ŠãŠ=+À?}"Pâ9©AAGN4FGL J0121.7+5153¿ÛÈEÓb¬âÀ%dí0µªÀ;'³ S\žÀ<ˆ §ªÔU@"€±ˆx´ó?úï'åJr?ˆZ!´†?À"ÈVñSj?÷V%¾@Ø!ÈýŠZ¿ïÿÀ	oëJ¿ïuÞ©n#?ïÿXJ¿¼sîdL/Ù¿ç
çIOÕ*?"™N›Ÿ´AGNbcu3FGL J0121.7+51542MASS J01213367+5155520?ïÿ	Ås®?ý½àcvr?ÇJ¿²V+?ý½àcvr?ïíÖ¿΀?d€${~[?b)@Óö/ô?d€${~[?ïðì®-i4?[œ7B\?^&£Uv©Q?[œ7B\?ïÉݘÉÖ?lÙbŸ^?{3—NÁ$?lÙbŸ^?ïþ;åçÙv?(%±™ƒ\á?,A¢8íu‹?(%±™ƒ\á?ï£Þ^$¸?£ ÄBGu?‡hqgþ?£ ÄBGu?ïæH#㽈?sŽÖŠZ?i·ÛðGx?sŽÖŠZ?ïS¶\?‹‹«î{‹K?•‰?œ\že?‹‹«î{‹KAGN4FGL J0121.8-3916?æ
"È=`ÀSyB=KÀ:¤ù8e¢À<›"´W‹@ "]8??ý"6÷
7?À—ða§dÞ?µ†
`:Ó;?öàÄn&N@qÝn°ŒÐ¿Öp¨ÿ¾Ç¿¥†K3/,¿Û¶\þˆ±•¿Ù›¨B›†¿æ'ø»h {?qs™;*AGNbll3FGL J0121.8-3917NVSS J012152-391547?ïþ›=ªý¼?7œ;–­?&L)|Ýå´?7œ;–­?ïõmR=åi?W ¼°Ä\R?U%[Îl½ù?W ¼°Ä\R?ï÷Ӗôv?@g/¤mü¥?PXÑ¢åþH?@g/¤mü¥?ïù\ºb‰Y?4·÷BÂ+?JÏÓáY?4·÷BÂ+?ïý'AŽ?É?)²"8áSI?3íõ§ªù_?)²"8áSI?ï×ýÊ=?uý¸ÎÐJ?ts'ïõ|?uý¸ÎÐJ?ïøõµ#bÜ?b(®§u2Þ?L)+Ê÷Mô?b(®§u2Þ?ïèÁ—åds?X>³÷Ã5i?g>hMuÄr?X>³÷Ã5iAGN4FGL J0122.1-3004?íï»ÀT©Ù¾L×IÀ;ä¨+,ÔÀ<ì·/¡®@#%oÑ@?÷jðSº'8@m}aT®®?«ßXVÍ?þú¢ Í¿¿ÎŒm?îÀÎۚƿéX•";"+¿áW7T*#À?™Á]=¯?ÄÙRíÞ5AGNbcu1RXS J012203.6-300507?ïÜþº÷?«2tQ£›,?~1€––l'?«2tQ£›,?ïåÿ!D¡?Œ|
^õü?jޘ@o?Œ|
^õü?%Ñ?¨÷šf)Fú?®‡_p®ò?¨÷šf)Fú?ïþHaåð'?/Åå?"¢?+yÞÚ¯?/Åå?"¢?ïý™^òdó?9ùÛ1ݖ?35¢YW!?9ùÛ1ݖ?ï¶27ú\?'Ü2#kŸ?'sr'jq?'Ü2#kŸ?ﱁöËßù?‰x;¾³?ƒŸ'Oo»º?‰x;¾³?ïì&•
?n³tSgoÌ?cÙ=PÉî4?n³tSgoÌAGN4FGL J0123.1+3421¿›ê€ÎçGÀ<†Â&€À:"Ž;—…ÃÀ<hÉÒ*Û@!¢Ÿ.ÙÝ,?ú~V²"<c?Àì²nì?œHÿ´øè?ßøüLl?@"dQ›©¿ìb>ƒÉM¼?ÐÛZV¢¿é̒ë)¯&¿™
?þÑ4¿ÒS^a_@'¿Ðg\…'ûAGNbll3FGL J0122.8+34231ES 0120+340?ïþÀe;n?è'ÙÔúÚ?#þ77]nã?è'ÙÔúÚ?ïõÙÁ&üC?TÒ9'0?TL}ŽK‰Î?TÒ9'0?ïóï"wJ?aW),‰?X ÷º•Ì]?aW),‰?ïþ+RǬ?B>‡Ý×?.mIÒ< ?B>‡Ý×?ïýxOYÚ?2bræãô?4?»¶L5²?2bræãô?ïÙê`Ôù?v@`VýžÄ?s
þL%çS?v@`VýžÄ?ïò"$Ã6?f÷vþë×?Z׶¥Žƒ?f÷vþë×?ïú?¹JÜ??<#hTüÞ?Gðå=?<#hTüÞAGN4FGL J0123.7-2311¿ßJ3æózÈÀTlÎþÖ4UÀ9ÊR:_w_À<-S±Wü@@ àÚu×È?ýmºßd?²'ØŸ¾Ì¯?˜™ظÏ{?è¹Nª@ø/Ó¯¿ð?ð¿Ü]aÚæk¿ÝI|`Mȋ¿àB¦¾EJ¿Ê¡½?6.AGNbll3FGL J0123.7-23121RXS J012338.2-231100?ïþ¿('!? 刐-?$
RSÅ? 刐-?ïó"E"÷³?dŒ8zHZ2?Y»uS‰x?dŒ8zHZ2?ïÕµçÍ?€Å3( ?uq%œ½M?€Å3( ?ïúçïRû?3z€¾žä?D`ñ3Oo‡?3z€¾žä?ïý²´âd(?,§Õۃ0?2jWŠÓÒ[?,§Õۃ0?ïȁéF!š?‡¨PÁŽ€6?{¿C';?‡¨PÁŽ€6?ïړy;w?€ an4ß?r¶C_"¦?€ an4ß?ïóÊÏ5vž?QÙ²T€0?XjaPZ"þ?QÙ²T€0AGN4FGL J0124.8-0625?ã62C@"æÀPõ7óŒT7À:"t•À<Œ›'8S@[ÅßȨ@'tý¾?Á¾«·ShÞ?¯Z"|ýŠ8?çi%}½ðç@ž•Ök‡
¿è[#aÙ丿䙅½nµë¿ãeØ!Ëå¿â²tý¾¿à}¯XGÀ¿ìÏñ¿öO¨AGNbll3FGL J0125.2-0627PMN J0124-0624?ïÿÄe©?
³ì¨)G?'zŧjA?
³ì¨)G?ïóÒ/bCA?Z}[oBP-?X[¡o³}?Z}[oBP-?ïùn'‹¶¶?6Å–'E?JE¹©SŠ?6Å–'E?ïÿ•¼À:B>öÀ¼x'ö?
Ý!`34>öÀ¼x'ö?ïÿ-(›ïN?FߤÁ‡¯?Zî	ƒT?FߤÁ‡¯?ïÌÉ)T7:?ƒéÖÙ¥'3?y›kgnÿ?ƒéÖÙ¥'3?ïúp}°HÌ?T ×_§¢G?F>	ɕ?T ×_§¢G?ïþÞ^^sí?(÷ŽGò?"é©g?(÷ŽGòAGN4FGL J0125.3-2548¿æÄ{'ûù>ÀT'†@ €À9Û7ƒ$OÀ<wÎaøBœ@NX"¿åß@&¸0]•Ý?¶Økš,?µfmrIHž?ýS
3_¨Ý@	Ò<m™‹'?ïšáBO°Â¿áŠ6ðW'¿à¢ªßè'¿âìeïH"¿é.xMïw¿ïþ¾P¤]AGNbll3FGL J0125.4-2548PKS 0122-260?ïü‹;‡ëq?2Ûßóx˜'?;¦%±Ÿ%ì?2Ûßóx˜'?ïó:[_?^çÇü5̒?Y‹ÍBq?^çÇü5̒?ïÛ(9|oà?v›Ô'Ñ'•?rkã1IðU?v›Ô'Ñ'•?ïðUs©?K{äØ»ãÃ?_Uþ°8Þ>?K{äØ»ãÃ?ïóÍz¥@I?Qɹ^¾Kà?Xe
"ƒ-:?Qɹ^¾Kà?ïÓÇ
¬L5?yꄼ¿mÒ?vy8HAr?yꄼ¿mÒ?ï¨äº.?‡•úÅÜØ.?…ÆÑyô|ƒ?‡•úÅÜØ.?ï×PÁ¹sT?e'7
ñw×?tWŸF1?e'7
ñw×AGN4FGL J0125.4+3200?éB{‹DIåÀ>O…r›(À:o€Ãþ¬À<\\3Ý}@륹¸rù@­"BJ'k?ö9¿‹P?ˆ?ºPVڂB@ÒL(!²,?ï½ö=	¿êÊáÛQÊοìNß+t"¿Ú%|ª¤¿é<¢¨6¿ïøHEéïAGNbcuMG3 J012541+3152?ïýO[)hÑ?7+ôŠ¶éÀ?5…(YÖ^ó?7+ôŠ¶éÀ?ï󳷁?g0FRújÁ?X™ÂÖ¡.[?g0FRújÁ?ïÊT%Wc¥?}m!Î'\
?zÕíV]ñT?}m!Î'\
?ïûßÁ5Û?/ÆO™¯{3?@€úԋQœ?/ÆO™¯{3?ïû̟Þà©?CÇî¶O)?@̀j¦±Ý?CÇî¶O)?ïÙ¯
@§²?uW"ÞiBg?s(ytIη?uW"ÞiBg?ïōÕYýç?­§èñ¬d?}9o-ØQ?­§èñ¬d?ïåñ=bê?`Ì´"o¦'?jÂýv/?`Ì´"o¦'AGN4FGL J0125.7-0015¿ïÿú‹™H2ÀNó¼ÓZ…ˆÀ:>¨*VàÀ<eŒÿWc"@ôÀÙú\Ó@T‹<߄_?ÀÆÀCQŽh?µOm¦v¡È?îʾ­	c?ü©NM?ùÀ¿ÎÈ^éooÏ¿êY9W:¿éµO!ü)1¿ìn•	 º¿ïþôœõn­¿ïÊO[–AGNfsrqPKS 0122-005?ïù¥ßçËp?IÞ[³ÿí–?IhªMhþ?IÞ[³ÿí–?ï¸jîDŽ ?"Ôóэ@?åDH÷n ?"Ôóэ@?ï€!k	¹<?‡ò›e#n?÷¥Dpèã?‡ò›e#n?ï…ú'‰ÿë?|
®ñp?Ž_ZiE?|
®ñp?ïÚö¨U.?{ÛüÙß?r"¬"´½?{ÛüÙß?î• ©vd?³U®¡'R`?¦­õk-sÌ?³U®¡'R`?ïkÜKu?Ç—¬û
a?'ž$xY\?Ç—¬û
a?ë7òãÀaã?²>ZŸ™ôï?à 4pþxt?²>ZŸ™ôïAGN4FGL J0126.0-2221?É&_<rïXÀT3 ù	kºÀ9ú¤û¨'À<^–ªÑÐB@
'èý/@Qè´k­?¸çý)áÐÀ?¼Íé'e"@Tá@ùòìòB?ïdcâ}Ž ¿åÄ ]Øù+¿æ58%á;¿ìŸõÔ-¿á:ҙ•gÜ¿ïý› Ø<ÂAGNfsrq3FGL J0126.1-2227PKS 0123-226?ïÿPWuï?ºþìÇÛÀ?üòðo?ºþìÇÛÀ?ïõ=Áxþ?ZTá­©L?U"}{÷_W?ZTá­©L?ïî:Ç7rÄ?c¤}'eïy?aÅ8§ü?c¤}'eïy?ïÿOfºf?ºL^¨üU?@rͪá?ºL^¨üU?ïÿu¼Ì/?
²ÁLnò?Hu….š'?
²ÁLnò?ïÕÌøìb?{\ꤱ?uƒ'Ø—C?{\ꤱ?ïâQZl6?qcßxÍþo?m®¥€"Ê^?qcßxÍþo?ïýß,±õí?%&ŽùØÝ-?1œ
».Å?%&ŽùØÝ-AGN4FGL J0126.5-1553¿ì³Æ̶//ÀSæ¯ÌâÀ;-Ù8ëÙØÀ<™Zž²O@9`<*Ô?ÿþøþƒÿ?ß±‰ÚÀ?ã=:ZMS?þ'PÀô*?þÝAאË¿ï•'¾´V?ã"; g~"¿å"]9–û¿é(ª^û'¿ïý}Ú rf¿ÑÓTÛúg:AGNbcuWISEA J012708.49-155554.1?ïæ4÷ÐÓå?"¶'AÉ]ˆ?iËq$š¾?"¶'AÉ]ˆ?ïÈÇÄp?‹Á£ão\¡?{œtŠã¡?‹Á£ão\¡?îÌJø2†?àåýX?£;PyoK ?àåýX?ãØ×ó?xªN+‰×?Žœ‡	ÊD?xªN+‰×?ïÕã|;ºÁ?xê½CZZ?uAü?§C?xê½CZZ?îª_Û:d?±Øœog
?¥ZHfÉ?±Øœog
?í³ræ7¾?Ÿ?'R‡¾#?²gœhÎB?Ÿ?'R‡¾#?ífŸ5(Æ?¨,m©Œe?·ËßU?¨,m©ŒeAGN4FGL J0127.1+3310?ì~§!ŽèÀ=~À¨À;MPïܹÀ<±­ÂEŠN@ wzÜÀ	ñ?ÿ:ŠÅÁ?Ñ?Ë)¬ ÚÁ?šúv~6'·?Ó°È_TÏ:?þù$f'¯j¿î̞ßS¸?ï—L¸?w¿ãþÊuÚx¿äWewS´¿Á¢@Ýîz¿âÛea-Â[AGNbllNVSS J012656+330727?ïþÞ¬ÀŠA?UÈAć?"5ɍY?UÈAć?ïóâL)¾?]ðNìN¬?X;g{	™°?]ðNìN¬?ïí…Æ'?]2¦µ|Ê9?bzã‰U÷?]2¦µ|Ê9?ïú4ÿ¼
b?4ˆÛ¸.?G,i7à?4ˆÛ¸.?ïþO_Iø®?#íì$?æ"?+
;þW?#íì$?æ"?ïËn?›ë?ƒwÙ5ñÁ?zHà5ã¦S?ƒwÙ5ñÁ?ïíû?É;?féçÁ2K?bÀûç?féçÁ2K?ïàäLMéö?eC´TÞ?o³Á4Q?eC´TÞAGN4FGL J0127.2-0819¿×¸œ­äîñÀQXh‡¨ÖMÀ9…(šRýÀ<>EJŒì@°áõ(
¶@ÒD}ÞR0?²¦¶¸ŽQg?¹	ÜÞÎé@ìÜ¢,æ@¦+
DÒm?ïÿá—_,¶¿à2f9Œê¿â?™s,Û¿ã­_I;³¿äÀÉë£R¿ïüäÝdʅAGNbll3FGL J0127.1-0818PMN J0127-0821?ï÷/âEÚÖ?E2ù—P',?Q ;¾äQ?E2ù—P',?ïφ{×P?ùÚ`®øn?x<Âx"ø?ùÚ`®øn?nûéÎ?†+êöuÁ?Šœ$:&Tn?†+êöuÁ?ï#õ'‹)â?ƒ~dF"ü‰?›M²
_È?ƒ~dF"ü‰?ïÚmèÌîÂ?q.™÷†‹?rÉ–Èï?q.™÷†‹?ï1†0?¬†uŒúQ?žyÝwÑ$?¬†uŒúQ?îŸÓOGæÉ?ŸÁ;üÒÆ?¦Ë
¥¬j?ŸÁ;üÒÆ?ìû‰Î b?¦@N€"Ü?¿@#±Šüô?¦@N€"ÜAGN4FGL J0127.2+0324¿ÔŽ=5ü¢dÀM ÖÓõ¶À9ëRV)ŽÀ<A¬½ã%@ª—mÅU?þƒ=¢!þX?¸–_×Öì?©"U´?òŸ£ž\w@XS­&>X¿å¶À'¢Ü¿ÁfA''–¿á,Xï
¿Ø͙ÞA¿Þ"â¨V¿âôN>aAGNbll3FGL J0127.2+0325NVSS J012713+032259?ïÿQpyÔq?D4C#^¥?ÑëÅ,eˆ?D4C#^¥?ïôtŸA×Ä?Y}ù÷ó'?WÁ/Y7À?Y}ù÷ó'?ïø"P‹x?TöÅ ª?OwíÜkÃ?TöÅ ª?ïÿ¢¬×B>ôûU˜ó²?Xœþ—<>ôûU˜ó²?ïÿJaçÀ]?Š´í€
"?³¾Z]×?Š´í€
"?ïÉcñÁùµ?ƒzž‡5-$?{N&m¡?ƒzž‡5-$?ïø«‡¿I?c|}»Q?MQÁhœÈ?c|}»Q?ïÿi˜±"ˆ?.Gáóµ?Ìì&Øé?.GáóµAGN4FGL J0127.4-4813¿à:ò†^˜+ÀPñ(Œç°À:¡îàªÀ<±HÒé4@6\>šD@¬u>p~?½¬Žé½Hu¿›íµ^\µ?ÝxÞ8/v@[–ˆB.?Š&Ã‰à¿ééŸ"w¿å¶?A´U¿á¤•á~4¹¿ïÿü¥¬¨?ïÿÍ
	n>AGNbcuPMN J0127-4813?ïûœñ	dz?;3ñÎÙ?AŒ<ãi¬?;3ñÎÙ?ïõó%•Õ"?Xr–Ñ5?TµÏXˆ?Xr–Ñ5?ïßÇR͂?sÆnCw?pu9šÿ?sÆnCw?ïþS{áš?$Ù~6Þ?*ÈM¯Tí?$Ù~6Þ?ïôÉdÇø?\yð¬_?Vm7Ò.}?\yð¬_?ïÛמ%ß'?sêEû',ï?r1½Øž?sêEû',ï?ïÒ`+}¡?'I†PÐs¿?vÏêbÛ©¡?'I†PÐs¿?ïö¦ŽZÝW?HÞe³.‡O?R²ã{¿°Ü?HÞe³.‡OAGN4FGL J0127.9+4857¿î×µþ¡}‹À*÷´ÜëÿÀ:9ƒ^ıuÀ<%'¡}"@ãþàEP@؝jßqë?½"¿Àéz¿*ò¿Gœ?Û÷ƒÈL
@v¢ÔUØ$¿Å/"Â͚}¿å"wvY"±¿ãNU}àÖo¿ê\ \–ÙÌ¿ëEMýcîg?ÖºqëÕ¦AGNbll3FGL J0127.6+4851GB6 J0128+4901?ïý°Ý'ýv?&аF¸º?2y_B?&аF¸º?ïõz<°?\ÑÈ;ÅâN?Uõn9ÏÉ?\ÑÈ;ÅâN?ïÕ,'GTl?yp®­î¶e?ui·Zõñì?yp®­î¶e?ïû!Ç®ˆr?/R³t5þ?Cxáù¥
?/R³t5þ?ïù£ýB,î?EΆPSÝ?Ip
ìÚF'?EΆPSÝ?ïÌÛ{néË?€Ö'2¯?y'B)žžŒ?€Ö'2¯?ïÊùœtÑt?'J—"zå?zƒ1ªeõ?'J—"zå?ïâWÆîïë?^(¦†¡Î&?m¨9O%
?^(¦†¡Î&AGN4FGL J0128.2+4400¿Ý/®|]QGÀ2^ê šª;À:ñJ¤iuÀ<gÕÈc@}"‹›)@2mæÎ?ÒÓJàxü?Þv­*@pZ:Þù@'N¤RÛ?ïùHUÚ'(¿â£«€ÌÄ¿é	¬AU¿å
" ®¡>¿ïÿ÷fÔJp?ï¢O¥YÁAGNbcuMG4 J012818+4405?ïÄp¥ã©?ªÖä2,§?}Ç­<[°?ªÖä2,§?ï®ÐêWú?"
3oC.Ô?"KÅ\]Q~?"
3oC.Ô?ï0žo†'?Š¸ãe­P?™ì2
Ãâ?Š¸ãe­P?ïs«E5
Æ?xÛ+-Ùî¦?'Š—\ÎC7?xÛ+-Ùî¦?ïÉÙ ÎIØ?' ?þ*7?{/³¨Î?' ?þ*7?ë—w7*?Åt¨nQ?Á£§¶##W?Åt¨nQ?ìÕqÁĨ?¨Ún«ART?¹Tw*ÍÁ¼?¨Ún«ART?é×5è*‡y?³ÕòO
:?È£(_Uâ?³ÕòO
:AGN4FGL J0128.3+5710¿äºôœŽZeÀ^ÒàD²À:…	ËZÝÀ;ö÷ÛnP@@Ê?SÒæ@f–DzƒT?ÀË0šÁ¸¿¨tæ†Ý)f?æÊÐê°
@6hk#d‰?ä?}ïD¿á©ýýÇA¿éÖ.u^Q¿çÀÔÁÔi¿ÄÚWåD<ñ¿äMHˆ/AGNbcu2MASS J01282987+5712494?ïýïû·,8?%¹ä?ʅ?0€ ÐÈÃr?%¹ä?ʅ?ïòwY†a·?eŒ)Ԛ¸‡?[Lˆ"~?eŒ)Ԛ¸‡?ïíæÎçÀT?p.s~§xÉ?b1Ly»c?p.s~§xÉ?ïýX&Bðý? f Mh}?5>ÌȗŸ? f Mh}?ïüDŠÉr?7µu-!ñ??Uۍk?7µu-!ñ?ï¿<ö;í?ŠÃìÐ䎩?€0ù¿Ø¨?ŠÃìÐ䎩?ïåYBˆÞ?t&:«½Rš?j¦½:¨Þ^?t&:«½Rš?ïë	°éþ?Zğà8B?düö^4Iy?Zğà8BAGN4FGL J0128.5+4440¿à&nSÅ¥À1±Û˜AªÅÀ;"|úÀ<ŸÍHÏD@'³Jß@£a™x?τ"ú£tº?ÒÁqºWC@÷~0‡‡@
^~\&q"¿ïÿ	ËZÜÅ?ïþ¹ä'¼0¿à~ø=¾Òc¿àéÔå i¿âËNÀŸm¿ïýjŽê/AGNfsrq3FGL J0128.5+4430GB6 J0128+4439?ïý‰Áñb¿?,!r'q=?3±îj¥g
?,!r'q=?ïñçªYìl?\ÃÂRëø?\0«3iø¹?\ÃÂRëø?ïÁ–Öw?{Óó‰ßÜ?4À3ÞÀ?{Óó‰ßÜ?ïï̂¾Ðz?D¬Q·±	Ï?`3}EOa?D¬Q·±	Ï?ïþ>Û÷¦Ú?)MK¼Ž'e?,=æÞ¥v?)MK¼Ž'e?ïÄÏJÞÿ?ƒ|Ô~RY?}˜ZˆñXƒ?ƒ|Ô~RY?ïÂ(RžLK?~×ÿc؁‰?~ëÖ«Zz¸?~×ÿc؁‰?ï¯ùðúÝ	?të2\ÙRÍ?"ƒÊ¯°?të2\ÙRÍAGN4FGL J0129.0+6312?³wO8?äÇ|Ìy1À9VÚÎO¨À;(Âñ·ü@)Ûp©‹@‰‰>ÃO?ŸIO@?ÑÏᗊ @"ßBñX?þ[^¸ù?ê|Iâ¢!(¿ÜJÐÞªDã¿è+b€=¿èr(;ˆl¿ïþSÝͦ?B§D}AGNbcu3FGL J0128.4+62572MASS J01283059+6306298?éÐ߁w?Ƴ.&j3?˨¼ûî#?Ƴ.&j3?ány<×Ì°?ÐWƒA
Û?Ý#
†Pf ?ÐWƒA
Û?éî5áŸ}ð?¬‡'Èõ?ÈG(y'??¬‡'Èõ?æÀÌ"á?°£'ß?z?Ò~gÖö=×?°£'ß?z?ӄ:fI¿?ÇósIùž<?æ=âýÌÛ!?ÇósIùž<?ª÷I
:%?¼ —åfe?îPŽ»o,^?¼ —åfe?ÍSVÿ–"Â?²…"'¾?è«*@wP?²…"'¾?±¥H"©YG?¢>Iw#jA?íËVûW÷?¢>Iw#jAMIXED4FGL J0129.7+3436?ïÈ}?çÀ;—{Zê1bÀ:ΪcyÀ<¢|(oŠÒ@©…©	¤?üYo!öÊÍ?Ì2T¦uu"?ÑèßZ©š@ÂE¿ý±q?ü;ÓÐÍŽ¿í^¨âŒÒŒ?ïÿŠ#ÚМ¿à?(¿'ÐͿێÅ?º«¿ã;½pcj¿ïþ2Ö!ªAGNbcuTXS 0126+343?ïøØÄÛDg?MUÆrÍøP?Lœë¤ã
5?MUÆrÍøP?ïløìñ-?™xΫ›»?'`â}jY?™xΫ›»?句¨X×»?}Û¨æFN?†ÞUâêÙC?}Û¨æFN?îé6Âß¹?WJxvï®?¡l"Õt!?WJxvï®?ïò곒"?TÛà¯æ^°?Z*™	''$?TÛà¯æ^°?ìBAã$?ÂtË
Úß	?½íðçfߑ?ÂtË
Úß	?ï&"³"¡?"n?Ia?›;©–•Aì?"n?Ia?êñ˜ß	?±‡ió?ǜ9œƒÙ¿?±‡ióAGN4FGL J0129.8+1440?…•ªÊå4ÀG"ÇŽŸj"À9ü¹w…r›À<UÍ&Žà@‹]†6@ø6Ã
¬+?¼÷¾=?Ňz]>J@8âe+Ô@uÏm À?áÛނ׶5¿äÄÏ"¢À¿ëSÕ£Ï(¿æü":µ´¿ïÿØ'sâP?ïýgr0õAGNfsrq3FGL J0130.8+14414C +14.06?ïñïYû° ?[Œ4Ÿ6>?\!KÃ珶?[Œ4Ÿ6>?ïíšcTIj?dïK©)
7?beœpNÀ?dïK©)
7?ïÅér<;?x IN}?}Gî†B?x IN}?ïà‹éá8G?\ ²HÛDÄ?otçÍù?\ ²HÛDÄ?ï£ð0e^»?‰J|i̼ ?‡óð÷%E?‰J|i̼ ?ï‡O—9dr?—`¢ÌÃ?Ž,;õ·m?—`¢ÌÃ?îè~'¼÷1?—•é"ë?¡x…sö?—•é"ë?îÏ.ñ|{ô?•ˆaÁn¨]?£
ç\YÃ?•ˆaÁn¨]AGN4FGL J0130.4-2129?ì7á.:{ÀSޞ²gÇÀ;8Ov_ÙÀ<Äå°Éa@ 90ƒUŠv?þK¡ô±î$?Ê,ëš?®.‹qYM?à…{ÕctD@xUy"%i¿ïø•½ìà?ïÿèþ†®/¿æ/:€.¿Ó+u¤œ×è¿àqÏP4˺¿â•=×AGNbcu2MASS J01302573-2128389?ïÿÇOVÍ?¾Z¢à9u?§Jý?¾Z¢à9u?ïñŸ
2(Ø?c¬ò0Cr¦?\Áå´kD?c¬ò0Cr¦?ïëãy¶ñ?n°mÚÊâ?d†i(G#?n°mÚÊâ?ïûVÍíW?,E}£Ë}?B¤ÇRԐ±?,E}£Ë}?ïÿNôÒä?ÅðÍ°Ýé?!_xL?ÅðÍ°Ýé?ïÌo½ä8?ƒGO7Tø?yðÈ=ê›é?ƒGO7Tø?ïòl-Œ?j…'ú†?ZÅÆÄ°(¾?j…'ú†?ïí0+Z»|?V(ßå[΃?bÏԋ'{ó?V(ßå[΃AGN4FGL J0130.6+1844¿êJõ¶ó>ÀE"C•%À:·t×Bq•À<zd׍@D§ú°`@؞wNëö?½£‰¤^¦Š<¿f?çm°r#3?ûÒÖ+›9W?ëÙßYí1¿ã¼§ñK1W¿èy6ýîü¿Ùö?¿æËxÚq3¿äã߸âµAGNbcuMG1 J013030+1843?ïü•á9|Š?,á>›Æ%?;PõCP­Ã?,á>›Æ%?ïéܯ×ú?j—…'\?f#Pûçµ»?j—…'\?ïì{¤n½V?^ž´È^}?c"['$b?^ž´È^}?ïÖ?ÊÓß?V:>Š"€?tàىlz?V:>Š"€?ï÷–Mp‰?J5QÒfH?PÓe0q
?J5QÒfH?廉ÐhÒ?‹GRHlî?†~OUg`?‹GRHlî?ïãœãX²ý?t!0‰5'?lc¡Í¢ç?t!0‰5'?îã'HÖø9?ˆ€-¼ñ?¡Æëq´•w?ˆ€-¼ñAGN4FGL J0131.1+6120¿ÛƒŽÇ"»¿ò¯bXº¬9À8Ê&LšãFÀ;™Ô	×ð@ œxfn?ú'ƁY0ô?«_§/"R
?´dsá½äk@mgŸKŠB@5êhi ¿ïìk˜ÕN|?ï5O؅g³¿ÒÑ@"ªt2¿Õ¼`Ï"½¿Ú\"»;*¿×fq#-×AGNbll3FGL J0131.2+6120RX J0131.0+6120?ïþ±ï%è?tùcÌ?$á7f/?tùcÌ?ïâ¡F€%?x*«µÉ¦?m^¹èÿ;j?x*«µÉ¦?ï¾¼.w¸?†Æ¡E§­m?€PýòRN?†Æ¡E§­m?ïö=é†{?>Œähf?S".3«9e?>Œähf?ïþ1voó?%¦KÆMØC?,è"ü–[ÿ?%¦KÆMØC?îë¦0½?²±}i<i?¡E÷ä¸?²±}i<i?ﳆrJuD?ˆ#øÐXÂ?ƒc{Ñ
ã?ˆ#øÐXÂ?ïçÉb?^$ëkü+û?h6ž¡ŽÍ?^$ëkü+ûAGN4FGL J0131.2+5547¿îúÓÎÒ>.À›œÆtÄÀ9Ѳ–À¡EÀ<Úìô‹@	²:zOQ@Ç>'Ä?¶)G!&Á5?' Cò7?ÚÉmÝ(9°?ðìÌKós€?ëÓåjR"¿ÒD¬{*C¿ä"éœl_¿á¢>ƒÉM¼¿áèi«•D ¿á?áíEhAGNbcu3FGL J0131.3+5548TXS 0128+554?ïõÜò΂ô?S¹ÛKrF¨?TF—4'c?S¹ÛKrF¨?ï¶ó†—U¿?Šc'}ن?'C^ú=?Šc'}ن?ï˼þë?wfÄʔ?z!§y²?wfÄʔ?îTOü0?'w4©zÄ4?ª¾Zÿaê?'w4©zÄ4?ïϽ\cЁ?wî™Ky$?x!QÝ6>?wî™Ky$?î%…HÀ'?µ­X.¾z?­§®lOäŽ?µ­X.¾z?ï¤)Ïv>?"+ÇöЉ¡?†õŒ,ËDt?"+ÇöЉ¡?è<~$aøÝ?±îQ;?Ïnx‹?±îQ;AGN4FGL J0132.7-1654?™`ñPÀS0#̎À8qŽ©{ŽíÀ;âêJŒM@»ãr€¦@&ÝA‰?œS蛛¡?¯" î@UL}‡\@:T‡–·½?¨­[ î*H¿âgwÞ]îÉ¿å"Â<Pg¿åfÿš6¿æ-À×K+¿ïÿƒ}ùUAGNfsrq3FGL J0132.6-1655PKS 0130-17?ïým"ùà'?-X JDa?4"Ùý­pÒ?-X JDa?ïóI4À?`UhÑËpI?YmÍbDÕß?`UhÑËpI?ïáŽóœù?uþXÕn†?nqøâg&?uþXÕn†?ïþÊâM"Ú?‹ÉLµŸ?#QÙL<ZÑ?‹ÉLµŸ?ïÿ£:=z?{¥þWåi?K™/ž?{¥þWåi?ïҖË^Ñ?ý
ê®!?v´š6,£Ö?ý
ê®!?ïãp1H©?xQ° Ê?lÏ2±ß?xQ° Ê?ïýQ•Q"ú?,È>)ŽYß?5sUJ±-?,È>)ŽYßAGN4FGL J0132.7-0804?ÖÆànÄÀQ%EŒÒ
úÀ:½%eëdÀ<{Y"M@ >_W(…Û?ü4sT‹r?ÆlN'^?ÂÌP{£`?ý9ƒ)Ì@?ûdÚ­‹¿ïÿù&Çë?ïüe@Ìxê¿«{ŒDg}¿ß,ÐÃ|l¿âªo¥Ó¿ßæ‹d͊AGNbcu3FGL J0132.5-0802PKS 0130-083?ïþh5üï³?š¢và?)|að/™?š¢và?ïےA­ì¯?yFÈÒFÕ?r6ß;tz?yFÈÒFÕ?ïí5ý+Ô?R•Ë1­Ô9?bÊ´?R•Ë1­Ô9?ï§Û:Æû?jó÷v€"B?†	1=JõX?jó÷v€"B?ïôbàx?TáêϗÜn?WÕ:UЏÐ?TáêϗÜn?ï"ÃÿHÊõ?—,0EÔ0Õ?ŽÏ;‹²«?—,0EÔ0Õ?ïÛš%ÁÂ?u¸¯îÌz7?rq²Ûñ9?u¸¯îÌz7?þb_à?•(÷þ¦O?¦¶PÚû?•(÷þ¦OAGN4FGL J0132.8-4413¿ïòÇhúÀQ¿!>>)0À:W]$žDúÀ<¬wD@œÒá¹ÃÜ@"¡ã6ï?³"jŽSš¿«¾Ùo˜g?÷ûƒ™}?üSÙÆÛF¿ÕéC¥ò¿ç5ø¿ßHƒ|vÉ
¿ãÒ. ý;*¿è›_Óû?Ðؗ;ˆBAGNbll3FGL J0133.0-4413SUMSS J013306-441422?ïôª]vê?W:0&ˆ0?V«EV^ûö?W:0&ˆ0?ïèŽ÷KÛ?v®«ìë?gqyHÝ¿?v®«ìë?ï§`¦!×?…VÅð Í§?†'Öm;k?…VÅð Í§?ïå/÷We?V<£?jÐä6rÕ?V<£?ï}Þ`¯(ˆ?‰ô¥€mþª?D3ëÒ¼õ?‰ô¥€mþª?óÓ:¿?"shíà?‡CÁ´N?"shíà?ïOgÚìõ?'xn˜èXi?–¶ë[{?'xn˜èXi?ï›s—?'372IÑ?Œ'‡ø"?'372IÑAGN4FGL J0132.8+4324?Þnr4¶ýÀ2ÔUGZ2À:œ½‡µk‡À<~ÝW^‹§@Ÿ™¯i·@|¦ˆÃ?Å覺YX?ÏèªäD¸—@*%£'·Õ@Q»úA¥¿êN›n…ð?×ò)é•ö¿æÜ¢˜E܃¿è6'@Œ¿ç¯§"X¼¿Ò6ÓfD¸AGNbcu3FGL J0133.3+4324B3 0129+431?ïøå³3Ú´?E[ÖoTÍë?Li2{¶+?E[ÖoTÍë?ïíTØ°–ò?`Ѻ-ŸÐ?b«'Sˆ•Ÿ?`Ѻ-ŸÐ?ïÐÓ߈Ã?jï!²qj?w–FúÞT?jï!²qj?ïË}lg\[?ZFÚîÅ8c?zAIÊB³?ZFÚîÅ8c?ïÜJàÁæ?t4åhÆt?qÚööáÝ!?t4åhÆt?ÿ2û€?•,}H'?ž€@ÿó?•,}H'?î°bd_aK?œÆãÌz?¤ùÙ½y‡P?œÆãÌz?îDm@±\??•s«£{Rƒ?«¹+õÆ#?•s«£{RƒAGN4FGL J0133.1-5201?æôþ>VIZÀOó'½RÀ8¸_b"À<Ûä—Ä­@a–8¼@ÐlÚ"?¡¹nÝ>›,?´ØœŽÁy]@}<y-ˆ@zdËÍ¿¸tsß²¿á%ĵ§Z¿åŒÙ݁zê¿äIê.Ýc¿ç-""aSØ¿ïÿGþò8íAGNfsrq3FGL J0133.2-5159PKS 0131-522?ïûÑãj¦›?:0b«Œ}?@¸rÓJx>?:0b«Œ}?ïöÜÒö©â?V—"¨['h?RFZWdjä?V—"¨['h?ïãaÿyr]?oe¦ZIJý?lžÃÂí?oe¦ZIJý?ïÿòáUè6>ÑFÕÍ¿>Ú=RFƒ?é>ÑFÕÍ¿?ïþþé~?—ËQ¼0? ?)
cO?—ËQ¼0?ïØB	Ëìä?€8å+ÕQ?sÞû˾?€8å+ÕQ?ïêŽ~)óç?skIép?eqæŠ90?skIép?ïÿìÔÿ÷>à0ېd>ã*ñœJÅY>à0ېdAGN4FGL J0133.2-4533?˖Bï`BÀQrŸ˜·À;·.Hè§À<ÿ'zç&ë@!Í\áb0?ìišÎM?å‹ÿ'=?åÓ°ìœuí?þëªX-¾?ò'.䬿ÙäŨ¹?í,{ž†é>¿í¤.}ÁÌ¿?ÒÄîý#VÇ¿Ö+ò¢xf¿Õ>ºÛˆ§YAGNbcu1RXS J013308.8-453528?îê笈E?Äø€±ã‰Ê?¡_±ˆ§¬?Äø€±ã‰Ê?ïÖ§ê?Nu?‰ã¸Õ&Á?t¬
ígI­?‰ã¸Õ&Á?ïQ=$M½"?Ë\@dø?•Ø[vH[¹?Ë\@dø?ïÛ
é¾Ñ?b†gQŒ©`?rz‹e'³?b†gQŒ©`?ïЍËýfj?€ êw{a?w¹àP‹&?€ êw{a?ï/R€«a?®èñu‡¡?š¯ç$A?®èñu‡¡?ïA´`¢àž?"õɒ¨:?—ÉsïˆC?"õɒ¨:?ï‡{jÀ¤\?‡¦®¤"ž?Ž!%SF…?‡¦®¤"žAGN4FGL J0134.3-3842¿å˜PDw9"ÀR֜wškQÀ:í—û3èeÀ<ÆÝåùÄ}@åçØkç@n£f¡õ‰?ÅEp!¦?ºd]þ7ÿ?ñ oÇ88V@-âÃJb¿ÎY	†'¿ÖZ–d
0¿çD[C¢¿å[«!Z¿ïý¶¿oA+¿ïþë-
$FAGNfsrq3FGL J0134.3-3842PMN J0134-3843?ïþÎø 8?!3Dž"e?.Vgk¿?!3Dž"e?ïö^Ž€¶Ê?VÈ䂚}[?SBãQ	7?VÈ䂚}[?ïÜ_ÿftv?k³…)"›?qÐGöQ<?k³…)"›?ïý´AVÂ?¦ß'=?2]õû!Ș?¦ß'=?ïþ'´`*ž?-(;{'‹?-"º«Àó?-(;{'‹?ïݯú?s5wÈç?q(?ikJ?s5wÈç?ïéoB>O?oGñ€À?°?fàž%I?oGñ€À?°?ï÷5ùiÁ?Cþ¶0Æè:?QœÈtM…?Cþ¶0Æè:AGN4FGL J0134.5+2637¿î8B]¨ÀA oÞµ,À9U"¢ß"yÀ<
:䜸@@‰°îIõ?ÿ@7þtÆ?±:Çw"?šTg¥™H?ésñ~Ý֊@EZ¨6¿¸³ÿÌS€¿æÀ|ôGe¿ãÚpßf,…¿Ï‹Íþûô¿ã7a@6ÑοâV¢8¤Œ<AGNfsrq3FGL J0134.5+2638RX J0134.4+2638?ïûD\®à0?9¯Æ's•?Bîô÷úZ?9¯Æ's•?ïô%:eñ:?X"–­²|~?Wµ‹ŽÓ:Ð?X"–­²|~?ïæ¶GÐ#C?rMäÎñ÷?iI·û¢¬Ì?rMäÎñ÷?ïäáі¶?VÎMɖa?k.Gpp?VÎMɖa?ï÷?ś]È?GVÏݼ¨¬?Q€t—Ê'?GVÏݼ¨¬?ïÏ<reçÕ?z][Òd?xaÆØ
Õ[?z][Òd?ïâ€W,Ü?vö‰2eý9?m¨±Ùd1?vö‰2eý9?ï°t;ˆŽ§?sº­x›~?ƒâñ+ò¼<?sº­x›~AGN4FGL J0135.0+5338¿é¢V"ê»ÔÀ!^3‹GÇ?À;&ԅ'òÀ<´¯L¤@#hŸ§@Kj¿'zç?ԙ¨}b+n?æý6Œ"a@×'j@@ñ#
Ì?ïýÚ¡K¿œ¿Åz‡Á…Ç¿áû3¢™Èi¿ëß3םá'¿ïÿú÷''ý?ä™'¥RAGNbcuLQAC 023+053?éÙKA--?Æ9Sð?ȚÒûKK"?Æ9Sð?ìcîÈ'Õ?À.F>ëM?¼à‰¾ÁWŠ?À.F>ëM?êeDPD™–?­Lªxp?Æjî¾í™ª?­Lªxp?ë—ëüèÉX?¡$‹Ôν­?Á P\Ú¡?¡$‹Ôν­?ߙ²0òÄ·?ÍÅ;'")ù?à3&熝¥?ÍÅ;'")ù?ÑÊë&Û?ÏJP
çý³?çŠl¿?ÏJP
çý³?ÔÍ@eêV?½ÐÅâš5î?å™_Íp
Õ?½ÐÅâš5î?Öç'¹Nã?·ÝS	'Ì?äþŒl#XŽ?·ÝS	'ÌMIXED4FGL J0135.1+0255?êó•I¹îŠÀM½º
RiÀ;w³Š§àÀ<­ÓÀÜÕ@"[ÌÚ
Òü?ùYÝÿôB?ÍoÃ\`©
?´~!sBB?éSme^(ª@(â@Q~οïþš9҉¥¿¹³BVä?ïüùðòF¿Öצ$lpì¿ïé
?ƒ£Ž?ïгâ;ëAGNbcu1RXS J013506.7+025558?ïþõ¦;? ÉI"¶7? ¯§v#—? ÉI"¶7?ïô¯yw1²?[UòÑrf¸?V¡
lRK@?[UòÑrf¸?ï‡À`#?…€ŽÖ~¸?Ž?ÏïY#9?…€ŽÖ~¸?ïúCê?=†>RǙâ?Gâòú½S?=†>RǙâ?ïÿO>è¯=?ËLöÎtç?+/P¡Í?ËLöÎtç?ïϸ]ÉÑ?{"4ªË~?x#ђ˜—;?{"4ªË~?ï¯E¦A7?†¾J™zg?":®†Iˆp?†¾J™zg?ïõS0ԉ/?S‡Gª2ó?UYÐ<ó@?S‡Gª2óAGN4FGL J0136.5+3906?ìuŠzåïÀ6ðMDVq&À7´åÏxyÀ;<Ðjæÿ@"n×S9?øû"}ö¦?š›œÂݤz?´û0f…p@Õèc+Hƒ@uU6=SÈ?ïû!>>)0¿Ë»Cs¿×Ëw!ʀ¿ÑW8 ,ñ%¿Ö˜Ç¢"¿âCÖNUÎiAGNbll3FGL J0136.5+3905B3 0133+388?ïԄ-:?ó9ÿ•?u½énfå?ó9ÿ•?ïf^È|?•É\0Ö­8?ˆ¦hC'$P?•É\0Ö­8?î×É]#?œº·g?¢Ž³kåœË?œº·g?ïfÜo­?€q©—œ?"$rxh?€q©—œ?ï¯C Tøð?…ù­:G?"/7á"Ü,?…ù­:G?íPCނØ?ÄF²ÈOöŸ?µ}çÂÄ?ÄF²ÈOöŸ?ïVeà.©a?—±·:eø?•3Cö»7î?—±·:eø?íFbvÙ?¤VØØ2i?µÌëz"Ã7?¤VØØ2iAGN4FGL J0137.0+4751?Ú:ÔBYcÀ,žß?–À8	wíwg@À;–ϲZZ¿@"58$t@'ßƤ"Ÿ?œºâ"Š;-?¹E6€o§@Ÿ
âµ@¹õ"¦î¿É8ÄA¸Ý¿àiˆ†a¿äªg|æÛl¿ã÷±j8X¿é!ÔfB¿ë|辚ÚâAGNfsrq3FGL J0137.0+4752OC 457?ïö_uu<?P?ûöq´?S@öØøt?P?ûöq´?ïç ®òØ`?v$_¯_Íõ?h_PðJçÃ?v$_¯_Íõ?ïÞUz¨44?r}ü]	!?pÕBÈž?r}ü]	!?ïþ6~cª—?!ÙY°q8?,˜Ž\Ô¶?!ÙY°q8?ïä›Ôø?aRÇùUxL?kd,Fà
?aRÇùUxL?ïð'"8?¥'4Îò÷?ƒùÛ^ò?¥'4Îò÷?ïÔ¡Z¶¸l?€hßƱK-?u¯R´qýï?€hßƱK-?ïù`S??ÛE)G6.?J…Oº'ƒ??ÛE)G6.AGN4FGL J0137.6-2430?î;)öTVÀSÒaAcwŸÀ9ɇî"À<BÎxžw@¿aj~#@@E®_ú?¨£,ëEˆË?½¨Ù'¤Þ@«c|§Œ@[òPêԿž¡{eQ¿ã2†óпçWã줩¿éž¥2¿êÌÝÿ$7î¿ïÿŠYŠµÑAGNfsrq3FGL J0137.6-2430PKS 0135-247?ïû£•NŽâ?=ʑQéÁ´?Aq«ZÀTq?=ʑQéÁ´?ïôG5@ ?\Ø¥Ú*êv?WÃq$̐V?\Ø¥Ú*êv?ï͎¸-ó?uʔˆÂ—¤?y8£é¶]ç?uʔˆÂ—¤?ïÿQx‡j?IåäF%O?Ðé"¼²?IåäF%O?ïý¬dç$+?)§ñt°?2œ×Ÿå?)§ñt°?ïØ¢R·Ý?uR4šWTß?s®ÖÙ÷EÝ?uR4šWTß?ïÖäO—º>?~üZ‹é?tØU í?~üZ‹é?ïþ%ý7@?#—Ñy«Ú?- ,z'tµ?#—Ñy«ÚAGN4FGL J0137.9+5814¿ïA/¹ðÁÀFïÃqÚ8À8Î3œ¾àÀ;ÊÖyù@ -ÐH'OÑ?þø–IƒÑ?¦ZßZÕ?Žà8±Ä«
?çé‡=G@úºÈ}Ü¿èQu¾sпԳµ'k€¿àħš
\à¿Ý
ˆïþ*=¿àÅ+<¿ØO*ÀH&AGNbll3FGL J0137.8+5813TXS 0134+579?ïþ÷žÔä@?"¥ë? †ښA=?"¥ë?ïóû¿qP?_CÐrr[?X'9'€J?_CÐrr[?ïîu­gh?rõP«¿c?abŠ)]H:?rõP«¿c?ïú>Íp?8ráé5$?G›ÓÌæ±F?8ráé5$?ïý`q–™?,¸K°?4üt<`V?,¸K°?ïºgaO"?·è×æø?f<µA?·è×æø?ïñj|†Êp?qa÷8R¤4?]+v¹0=?qa÷8R¤4?ïôpú¶as?MãŽcD ?W
'¾úe?MãŽcD AGN4FGL J0138.0+2247?·Åbª'³ÀCi:2?îÀ:%:G#«À<R÷eýŠÛ@²xà;"@}æOU?¸6Îs@–?q8áh¨E?ºS²ÚˆL?@z÷NU£?ì³åªê#ö¿ç^æªÄdH¿â ÿõEq¿ÖÄÀŽÐ軿äy-Œ*E¿ËgIû¡¡{AGNbllGB6 J0138+2248?ïþÔñ"[c?'ö#hQ?"°ðƒüE?'ö#hQ?ïõʬk-?X%0µ+OÍ?Tkã$|?X%0µ+OÍ?ïûBð%ӊ?/Š©A¥b`?Bô>æg
~?/Š©A¥b`?ïþ{òzím? 34ÍMÙ?(@ÙY*Ê? 34ÍMÙ?ïþÌÈ+c—?G*$œx?#3z 
?G*$œx?ï×y@*3ý?xÀ"=
ã¹?tC_çveE?xÀ"=
ã¹?ïýF¤ÿÿ)?>ï¹Ãâ-?5ÊÚ%È3?>ï¹Ãâ-?ïý"-'*,?##z6߆?3f•€ó??##z6߆AGN4FGL J0138.5-4613¿í¸";¥ŒÀQ0DR?gõÀ:j&Ñ%!"À<¤×%+3@îrì û@î¨|‹kÙ?¹õìUÔ?œ'Ý<Ü?ãªJè\?øs™)Ý?ïï
3Å)j¿¹ß#¦@¿çǃ·°¿Ù@X *,y¿à9¢cÑ¿ê	Ý>_SAGNbcu3FGL J0138.5-4612PMN J0138-4614?ï÷êîÜþ.?oþr"RoÄ?P*"c³v
?oþr"RoÄ?ïê"Ýí(?pvÖÔ>,u?e{"IѼ=?pvÖÔ>,u?ïÍaÖ
?€ÝÐMl³?yO|‡=‹!?€ÝÐMl³?ïÕÝ´ùG?`õ](ë?u%©t8z?`õ](ë?ïõeí<%m?QG¤™NÞq?U4%³°&'?QG¤™NÞq?ïµ²‡"Ì·?"*lÝpUu?'"^-"$J?"*lÝpUu?ïÂ&E¾?…YԂ"ÇS?~óì¿8"?…YԂ"ÇS?ïIñ~e"7?'æs–s?–ÁÐ.&&?'æs–sAGN4FGL J0139.0+2601¿àώP:UÀAϋ«`kÀ:´•ë/³À<8;-Ówâ@@,ôÄ0@"ÅDBO0?Í_á'¿'Õtß'¡?Íw,‡G‡~@¡¤ì³òá¿ë>øcSŒo¿à_*g²–Á¿Ûétƒ	µ6¿èBÜôb=¿àÒ\XÆ¿ïþ­…èÝAGNbllWISE J013859.14+260015.7?ïþ]–32²?#yzp$p?*&œ'ôö?#yzp$p?ïöZ·}ý~?U7^X«]Ö?SJ'qø'î?U7^X«]Ö?ïàEÀÝ?r»á®¸e?oº?yÔ&?r»á®¸e?ïýÈB×ô|?:àjŽÒÇ?1½ëZ'?:àjŽÒÇ?ïüñ׍	?5XÆ`/aƒ?8qCºç(°?5XÆ`/aƒ?ïÐZˆ..´?Ã-y¦XF?wÒ»óçeü?Ã-y¦XF?ïÓ1éËÐ?€¾WýŒš?vsç'Fãæ?€¾WýŒš?ïô»Î?L®ýÑZ—_?Wވê%tm?L®ýÑZ—_AGN4FGL J0140.6-0758?ë'má@2†ÀPäýó¶E¢À;¤ÍªB^À<™€'a–ô@ ÁŠ^"3N?ú¦¯ç¹¸?њ'ÇÅý?¢nªW¬å?óÝ­ûPm×@KŸ	0¿ìèiÿ#â?Ì:OMw¿×wS´Eí¿à­'f¿½›Á'¿êøC""~AGNbllRX J0140.7-0758?ïÿGԈ‹ˆ?	ôÒ¾–•?pàÛxË?	ôÒ¾–•?ïô˜l¯?`›ÿñVŠÌ?WüÏDÞm¿?`›ÿñVŠÌ?ïðõ'
¦?d¦{©ímb?^ÑN—â½?d¦{©ímb?ïý¾–B
?bÒ6[ð5?2Lù5M¶?bÒ6[ð5?ïþr'2¨?&è
·Rƒ#?(×Ûÿ—w?&è
·Rƒ#?ï̚'ªü‡?>œz?y²·,'€^?>œz?ïê%¢×?qÁP]Ì ?eÚ^/á5?qÁP]Ì ?ïøÁGÇ?EÜhê°Ó"?O´ûBCo?EÜhê°Ó"AGN4FGL J0140.6+8736¿â
ëøm@8ÉÒ¿UÀ:ҏØO·ÎÀ<A(¿<@ ï>fÃ?ÿy)L)¤>?Ç)×iÞÀë?¾ä0ì†ü^?ö®×ï?¾@
ç¿P7zì?ï(šÞ"ԿۏÔ>0<^¿Úõt,öƒ¿Ü/ö$_¿æ¾­OY§¿ÑHÈÆ­ÎÛAGNbcu3FGL J0139.9+8735WN B0126.6+8722?ïþû¡T+¯?$gl? Eêvæ«Ë?$gl?ïô6n&Ç?YáÒóvg?W"ÀÖ»3U?YáÒóvg?ïøu©ò¤š?Bfr£.ú6?N)XBÔ?Bfr£.ú6?ïõsC2s‰?6_°]š?Uyoí@?6_°]š?ïþÁ5?*^0z)?.Ï¢'<§¹?*^0z)?ïÍožbE?¼
¿]±ã?yH0ÕÇÇ?¼
¿]±ã?ï÷CŠæšÌ?ehiG¿Ï?QxéëR‰9?ehiG¿Ï?ïáìd
ì?V—Ž~<ÙÁ?nìdûSß?V—Ž~<ÙÁAGN4FGL J0141.4-0928¿ÙÔÆ`¢GÀQ1=Ùb·À8wŒE@ƒÀ;¯p"½'Æ@?mà-QÈ@²ƒ\@s? Nší¬–L?¨]ã#ë@ò*ڟg@0;'b|¿´#ŽûZÿ«¿Ý¡+>E[¿ãÓþð5ˆ¿âh·¿I~¿äàӟ¤Ë|¿â#*!;¹êAGNbll3FGL J0141.4-0929PKS 0139-09?ïþyÊ
>Œ?2Ÿê°Í?(cc}Ò+½?2Ÿê°Í?ïó/ébëÄ?aÑ&HH?Y -sáè(?aÑ&HH?ïìc½¶ü£?m¬×f¿3Õ?cœBIí?m¬×f¿3Õ?ïÿž—o>ýoÆÜI'?| 2û8Ð>ýoÆÜI'?ïþÀRZ°?Ý	À§P?#þJ€,?Ý	À§P?ïΞÇ­\?z2ÿ¸ˆ?x°û£Š?z2ÿ¸ˆ?ïçÄ^X×?qQN.¼ì?h;¡Ø°¬?qQN.¼ì?ïÿqåã?	SW¯Šíš?ÃXøcê`?	SW¯ŠíšAGN4FGL J0142.7-0543¿âküc¤{ÀPWÁ~ºñÀ;c1'À8À<±ÇÞP'Ï@JB•ü¬@3çÞ¡
§?Å?Ò(z#?ªqáÄ«–?äuòËd@Yï>½?ï÷®»iοä¿<Uñ¤¿ãʶ!œÁ¿è´¾c'˜¿Ëšã†!¿ïÿ~À¥L*AGNbllPKS 0140-059?ïþó•Zçú?Ya(-s? ƨ¼áŽC?Ya(-s?ï󁢵²?`eË<{Ë?Xüºýt»æ?`eË<{Ë?ïòxѲÔ?_كšKì£?[ØØLFz?_كšKì£?ïþ¹%ûè?ßÖ¿™?$m¤B=()?ßÖ¿™?ïþ£æƧ?!%ÐÐ%)ó?%Ï@>¼WÏ?!%ÐÐ%)ó?ïωÉ¡º?'VicÞÜ ?x;d€wP?'VicÞÜ ?ïéÊ3õÈ?qæ$j£ ÿ?f5çõE‡Œ?qæ$j£ ÿ?ïúûÛß?8Hrö¶$`?D‹åJ¼:?8Hrö¶$`AGN4FGL J0143.1-3622?ÊîÛ%2rÀRê–=Ć­À:Ìí¨À<"±ö‡±:@?þþMMf@qßƤ"Ÿ?¶áÓÞÓ¤F?»Æñ@Ÿ'g@.eÙx¬º@Q)¶1Õ»?ï÷XÇAr'¿åÀÇ`QN|¿ç!¼¿ænBÓº&Ø¿ìqT h«:¿ïþ–=Ć­AGNbcuPMN J0143-3623?ïý‰ˆš?%ýŠxÞ¯{?3·\ýe?%ýŠxÞ¯{?ïö*»â¼?Y\UúU*?Sª‡Ò­
?Y\UúU*?ïÛ½}.Õ?vV¦@£3£?r!r´Z¨?vV¦@£3£?ïÿ[äù?}¯ Ë?´˜Ï‡b?}¯ Ë?ïýúJo¡	?(¶`aÚ?0-ªæ¦›=?(¶`aÚ?ïÝšØ'?s€àZ‰;?qvðT?ã?s€àZ‰;?ïÔ5ûu½Ø?ÖòÃ<?uåA±wÈ?ÖòÃ<?ïýŸ$óÕO?%‹^¶€I?3Öª¡h?%‹^¶€IAGN4FGL J0143.5-3156?îg,"âqéÀSköU\RçÀ;È~‰rÛÀ<´Zåÿ£º@Eöê,¯@E]D~µ?¿"/?]¸î¿·(p«¯Ç?öî |wJ?ýàÆúOçÊ?ìÒvÅY;¿æ2eByø¿çÅÅqŽ¹¿çš×Q‹
¿ãµíB
@°¿ïø:¿¯#AGNbcuPKS 0140-322?ïý8!Pÿï?)ñ½Û4õ?6>ö&Óð?)ñ½Û4õ?ïۃ{lR?''q£H&…?r>B^]ÿ?''q£H&…?ïÛø»Vòo?h£æ%À?r¢>‰H®?h£æ%À?ïíµ›`vÁ?JÁõ‹ =?bJdkO/n?JÁõ‹ =?ïûÆ¡öœ?<ÊVÍ"ʉ?C¨åœúû-?<ÊVÍ"ʉ?ïm;¨ÞÂ)?¡P ×P‰Z?'XŠßPê?¡P ×P‰Z?ïÀ-%8Yõ?}k Eƒ?émVā«?}k Eƒ?ïEëÑÂ!p?‡K‹¸"+'?—B…Àܚ?‡K‹¸"+'AGN4FGL J0143.7-5846?Á¢Ìύ,µÀL‰A|¢À9	ëîÑÀ;òˎkß@/Y®2'?üz}Å'¼Ý?¥%þþ^{?¦Ì7ógä@n:p>V@Çc,Ë2?ïüX`iLJ¿Ô["©¤¿Û÷cÏ2X¿ÜR²à£¿ßŒ.Â5D0¿Ò6ƒµ+ÆWAGNbll3FGL J0143.7-5845SUMSS J014347-584550?ïþC£÷?_´Ó=Hš¬?.ïy ?_´Ó=Hš¬?ï÷@N'Lª?R[Õ*¡¹®?Qcæï?R[Õ*¡¹®?ïêUä™9?t·KC'×T?eª;ÿnb?t·KC'×T?ïüºÚˬÖ?)ƒ\õ,"?:)*ƒÿ®í?)ƒ\õ,"?ïþˆœz
?!¯(AÉ?'w)¡bIê?!¯(AÉ?ïÜIÿŽ§?tz+aMü?qôÚú¹Ln?tz+aMü?ïàå'ö?|Ǫþ`¸?oÿ÷¥Ë"?|Ǫþ`¸?ïú´"Ð9Ç?8ƒB"'M®?E-¬ O–?8ƒB"'M®AGN4FGL J0144.6+2705?â'ààUÚÀA%ú](ÐÀ7¢½	á*RÀ;[.ÿÇËÜ@‡âÏmý@C`Ðԙ?•s‹½ãÐÊ?µ€À)¦@ â ÊæBÀ@K)<d_P?œº×+öS¿Ûü@Ã>®'¿âIÆ×p•¿áÍE˜…¿æÒí­íäu¿ç³Ø>ð֗AGNbll3FGL J0144.6+2705TXS 0141+268?ïõ‹µ'ƒ?q­³·'ú?Uèè÷ѹk?q­³·'ú?ï»Çšë?'xnæ7þ?:Ì0?'xnæ7þ?ï¬ÓSÉ?Š˜.{»ª?"Ë?ÝOKÏ?Š˜.{»ª?ïÁê÷ìFv?p×ÕY°?ä?
ƒöžõ%?p×ÕY°?ä?ïíÅh)Š?`¸Un¶à?b:—èSåÕ?`¸Un¶à?8ª7ï?·ÛXçö-?¥Õ,v8h?·ÛXçö-?ïÅ´Á¬÷ß?‡ŒU­>c©?}%ŸF@"?‡ŒU­>c©?î+æÉßB×?HŽ[šQó?­A"a/ëŒ?HŽ[šQóAGN4FGL J0145.0-2732¿Öù#Õº"ÀS†KâCÀ9Xy˜rR-À<^ûE†@'‹öî´S@×EB<?¯½dác'?¸ÆÌ,¾Ïß@Ï¡·uM@ÉñS"ÒŠ¿Ø?$=È¿ä¦$Ÿòy¿ç»Þ¯¨Ð¿ê˜£?_¼S¿ífà‰Ã
¿î½Þ¨v¬AGNfsrq3FGL J0145.1-2732PKS 0142-278?ïþšÇŽkà?@"ƒÄ?&S†-;?@"ƒÄ?ïõ¾ÓÝ/?Z¾4#`;Ü?Tü'O£?Z¾4#`;Ü?ïèŒgƧ‰?^½-m¯…?gs˜m'‡.?^½-m¯…?ïÿóðþ}>аôì¾ø>ØȽ_7ó>аôì¾ø?ïÿF‰7ˆ?ò…j?×.áÚÏÆ?ò…j?ïÚQÞL¯?s…AÚ?r×Å
Ç?s…AÚ?ïáºc'u?q ØÎU?nüEƒÀZù?q ØÎU?ïÿ÷Ù>Ý5îêF>à^ùÏpô>Ý5îêFAGN4FGL J0145.9+2319?êq a}ïÀBì앿ðEÀ:ÏÓØZÀ<[‰2CI+@Ýyý@žÉý³ø?Ç·.jv–_?·jªÃ¸|?îzÜ?0—x@8'ÁÞÝ¿ã7=N?(4¿½x³š÷'ž¿ç=Fý•lŽ¿çLƂ/ð‰¿àɺ^5?}¿ïþP§ETAGNbcuTXS 0143+230?ïþis>Å?/‡'i—5™?/Ie•¤na?/‡'i—5™?ïó¤T³‹ˆ?^¡y,QÆ?X·V%v8?^¡y,QÆ?ïíè6iB?Y<Øç¬?bÉÿt¶'?Y<Øç¬?ïù"Y'cƒ?2àa}4]Ÿ?Kv™§Ô|ù?2àa}4]Ÿ?ïý™å³'X?( ŒÏÛ«b?30Ñ3ö(_?( ŒÏÛ«b?ïÌâ;bÆ?|ŨږòE?yüû»¸«?|ŨږòE?ïÝ4˜&ì˜?wH|¡^ZŽ?qe³Ì=`T?wH|¡^ZŽ?ïÓAàÂos?gÌB'ˆ«C?v_¡‡ök?gÌB'ˆ«CAGN4FGL J0146.0-6746?ï¼ÈÒä‹RÀHBòù‡?ûÀ:$"çƒ1xÀ<"Ö«rßñ@#¿ÆÿÙ??ÿD¶Ê,	?¸\ǁ3qG?¾E¿&ñÜQ@·Üz¿¹¿@|š	Öîd?ÚÀïÿÕÙ¿Êèà©£}¿Ûú©ÿÿáр´¿çÊäÊðS»¿àów[0AGNbcu3FGL J0146.4-6746SUMSS J014554-674646?ïþ²©ú©™?ˆ€-ä??$Õc3ß½á?ˆ€-ä??ï÷7†Ô?RC‡/Þæ½?Q÷'£î?RC‡/Þæ½?ïóÝ)]¾Ä?V­Ù:ï?XE­p}vç?V­Ù:ï?ïû:Æû?+òrÚXGµ?CçüaJ9?+òrÚXGµ?ïûÙïíZ®?D|ÄðÈ®¯?@˜@ÝP?D|ÄðÈ®¯?ïÜïÍ,îö?|`ÀßA…?qˆ`™ˆÖ?|`ÀßA…?ïâ/ÏÀ6?u€xÔ.ÃE?m€ÐaÒ?u€xÔ.ÃE?ïôaöÅò?Dã)Pµ€?W<xn¸,Ê?Dã)Pµ€AGN4FGL J0146.3+4606?å¢Ì¢ý½ÓÀ/j²[1~þÀ:ʄս6WÀ<"Ä'k§ï@VÖüPž?ÿå€éŸk?ÇD×àÒ\?Çaá†îQ?ý¹áˆE´??û™R.v
?ïäY!bü¿Ñ²mÛ¥­¤¿àQøPV¿âÌÅ«p[³¿ã%™'¥R¿åAmž%øAGNbcuB3 0143+458?ïô•4lŠ?Q–¸'§èµ?V՗×æœ?Q–¸'§èµ?ïÇ(ʓPn?ƒ¯Ëñ˜Ñ£?|kš¦‰•?ƒ¯Ëñ˜Ñ£?ïÏ=Ã!"?tÚRÑDý?xa‡ŽW?tÚRÑDý?ïIä¿Kž©?qͤæbJÒ?–ÃhŽí?qͤæbJÒ?ïåø	'y:?dxNb?jöy…†I?dxNb?î'Äø0íx?«"Š£ìà'?§Ó°"Ý"?«"Š£ìà'?ïbÖ/æ¼Q?'Mmî5C?"¥:OßÛ?'Mmî5C?ì)úû^[?œÇåùk?¾·¸(%
+?œÇåùkAGN4FGL J0146.9-5202?Ô~¯9‹ÀO~÷üü?À:aØ›ïµÀ<!Õ<Ý×@h <K	ê?ÿUûµ¤a?À®I)ʍ?½>[/{˜¨?þ"T8fxÛ@P×8`™ž¿ëc>Ò¤?ÇA»Y¿á»Ëǔ¿ß¥áË·y¿ÞËSûÕ£á¿ïô`{?çAGNbll3FGL J0147.0-5204PKS 0144-522?ïû¶ÄšÀ?<&¶8´L?A$íùý¢?<&¶8´L?ïïÍÞa—?eýà!‡žù?`2ðáÁD?eýà!‡žù?ïå©·àÓ?m‹6Œ$'>?jVHì?õ2?m‹6Œ$'>?ïåë‰ÑO"?Qà²3K¸a?jvrÄ<?Qà²3K¸a?ïôŒ	kÂ$?QÉWíTh?Vçì÷Y<?QÉWíTh?ïÀ&?—½?ˆÁ²üÎ?ìþýÙa?ˆÁ²üÎ?ïÆ
æ/kË?€Mƒä'¤?|úŒÅîÊ?€Mƒä'¤?ï{üfS­7?oýó/¹?€s>!_?oýó/¹AGN4FGL J0147.7-1321?ïŽ6텈ÀQ½×¡<%JÀ;i™ù:éáÀ<ÐI4&x:@Ë{uÂ#ü@Œ¶â¼y?Ú#<E*¬|? ú¶j	ß?Ä¦ý/k?ÿÀN²º¢?ïú
'Íx¿èå).‰¿â;¡–¾¿Óšß_ ¡á¿é~lLYtæ¿ïÿúŒ"¸'AGNbcuNVSS J014804-132019?ïø½Ýà_@?AA?\é=?M‡ñ9xÁ?AA?\é=?ïñ+@BØ?a#¢ûLÑè?]©µ«¿ª?a#¢ûLÑè?ïÍ×ú'xë?v©?îDN3?yèÓîž?v©?îDN3?ïôÎËÏ??•3ÓÌX?VädEàA??•3ÓÌX?ïôäVèUP?TKåØˬf?V7QÁaáQ?TKåØˬf?ïÐ%äÉ¡?x$¯x-W4?wôíO?x$¯x-W4?ﱧ)Ð?…&ŒO¼ÓF?ƒ–5‰>J›?…&ŒO¼ÓF?ïÐñ•ë"?ex¿6
¼'?w‡5PµÓ?ex¿6
¼'AGN4FGL J0148.2+5201?ïY¶ØðÀ#¾åGÆÀ9³EB<À<!»¹@ ¹%ô†O:?û^SEÎ@?´lŸe‹u?¹—½÷FóÚ@Tù¯ƒç@FI»_è¿ïýè~;?ïÿõÿ 1#¿Ä")Èü3¿ÜX
Ã}m¿¿Û¼ýÌÉó¿ÕÅi@¶SAGNbll3FGL J0148.3+5200GB6 J0148+5202?ïý¬ÙðÕH?-4q+ZÃ?2™1÷÷B?-4q+ZÃ?ïæ¢-IB?q!³‡Ã	«?i]úµ¹?q!³‡Ã	«?ïÛµ#t	£?yjŽ<æß¡?r%n<\Fd?yjŽ<æß¡?ï­¿ÐÝJ?hI½ýëÂ?"ÒüN¶?hI½ýëÂ?ïù½£0""?Fú•t.Š?I	s)Zj<?Fú•t.Š?ï]ÿW8¡?§	‰R?"@|C;?§	‰R?ïº\P ?†|áº5??y¨ù¹?†|áº5??îÄ|<>s?4êj™ê?£¸<:ü|Ô?4êj™êAGN4FGL J0148.6+0127?ïºrahÈ
ÀM"!ÄuæÀ:q'ùCM]À<e€<ÑA§@T˜Û-¸ @Ê¡C²x?·­®¤m³¿­Œ^Æù"?öq?|Ì@Ãú³ºØ?ïzÁҝÇ&¿èmÎÜd¿ålXï
¿àæY›|Ȩ¿Ù¢†,Ù¿ïú?̞©¤AGNbll3FGL J0148.6+0128PMN J0148+0129?ïþ`IR?ë@Ã<6?.)þ®°i?ë@Ã<6?ïóÓpø2#?[W꘩Ëf?XY>VjV?[W꘩Ëf?ïó¦ÿ™äÔ?iÇõ­Å?X²Ôug}?iÇõ­Å?ïúb'(Ô?-ì	³Ñ¾­?Fwdcß	Œ?-ì	³Ñ¾­?ïý5àÀ?-X_HÇ?7_|67A±?-X_HÇ?ïË	Bٜ?€®#Òâ¢?z{_­Ô?€®#Òâ¢?ïòÍ	ˆ"ä?ou'ó
?ZeìÍÙ÷2?ou'ó
?ïáïoþ¯b?^=ƒŸ(¯?n4*Õó?^=ƒŸ(¯AGN4FGL J0149.6-0734¿ê¥ue»NSÀP… …±…À;L;æ`ÊÀ<§Ö»cý@Eûxö@Èïþ*<ê?ÒEè8¹?ÃØEç?ê§?ñ"ì~Bûþ?úü,ý~?ï³@S'D¿Ë»5À¬-¿èåTƒ¿ãÅ©!ÌÙb¿ïþ
¡ÿÏ¿ìRÍAç«öAGNbcuPMN J0149-0733?ïò@Á³‹€?TJ qâ2?[~|gn¡?TJ qâ2?ïÀ½Â:D?™®'¸"?¡ïìxð?™®'¸"?Õl"º?f(Dîú¦?‹•
²™Ap?f(Dîú¦?ï' iàw?qr@Óôx&?÷ïÖ¶1?qr@Óôx&?ïäÓÎ/	?goøÛ+?kî,"gm?goøÛ+?ïJL
?¦É^Ò?ž6½ÄU¶¿?¦É^Ò?îß×ìï	Á?–¼à¿Ÿœü?¢03|ï?–¼à¿Ÿœü?ì¶ooY»? ì5#H?ºL‡d…2&? ì5#HAGN4FGL J0150.6-5448¿ï_†DʂÀN%db€'ÙÀ;K¹Z)ABÀ<ëªfpw@ #Œ¤ÄS?ùÃԅþ²"?ÓñýwŠ%?Ï*y¦41¶?ôm3	AÈ?ýî¦un¿Ò‰÷Dðtó¿êÖc"3ÖÇ¿ßü^ Ia¿Êç‰¼'¿çÕT{ç¿Àψ=üÞAGNbcu3FGL J0150.5-5447PMN J0150-5450?ïûLð?dØòõ&om?C¢ÌñÊ{9?dØòõ&om?ïóöŠ
…j?Y6kПF'?Xë±;¼7?Y6kПF'?ïØêùn҂?nÁ00ÿ7<?sŠƒTõW?nÁ00ÿ7<?ïô¾ åi?=§ƒá·?V'¾˜Ïí°?=§ƒá·?ïü_Ê?ÿŸ?5%?çrŽN?=¯§RâÌ?5%?çrŽN?ïЦ|'3?~¨Ê£J?w¬ÁÎCÕÐ?~¨Ê£J?ïÜÅùÒr?tSÆÊM£?qöz©=?tSÆÊM£?ïÓ@çRn?iwRVjï?v_ŒUÙéO?iwRVjïAGN4FGL J0151.0+0539¿Õ3µ¼1kÀK—þŽæ¸À:Á'ï2RÀ<mwVx²™@ӀÖ)Aî@ßûH
ZÍ?»ϘY'º¿²à#–³
Y?øq‹'æÎ×?þRP6ú*?ïú¦$¿ëÆíàBËW¿çt‡>.¿ÒbÌéR>'¿Ú§½ž±†u¿ïÿülòAGNbcu3FGL J0151.0+0537PMN J0151+0540?ïûW]ά?4U钭ëô?B¢‡á¶r±?4U钭ëô?ïã
`2<5?uÑ˸kw?lòŸ£(£Š?uÑ˸kw?ïåôÄbè?eŖØã?jàCÜ'¦?eŖØã?ïéŸó"§?PT>^a"û?fè`!	_?PT>^a"û?ïôõÓè[?PakM™êÔ?Wð&´éç?PakM™êÔ?ïšéˆD\¦?Š°ÒÙß?‰Eè	žw?Š°ÒÙß?ïºáÊ#¾æ?"½Ùk õÊ?Gsø '?"½Ùk õÊ?ï'½i¡@?Œ‰1ã?›RäóAþ?Œ‰1ãAGN4FGL J0151.3+8601¿¥gÏ6Ó^‰@7GM3H,À:´4çhÀ<h23Xòà@b¡…vL
@BLƂ/ñ?¶ ß´*·?‰0QxåçG?θÐV<<@Ee*§¿çIpŒZ¿áoáÐêê¿çÞl²[¿á['§åŒ·¿ç;ØÞ¨íJ¿ØÖ^¤ÑAGNbll3FGL J0145.6+8600WN B0140.0+8546?ïþYĎÝ?]`n¯Ôý?*cµvödY?]`n¯Ôý?ïôáìø	?Y¨W\¾3
?V<%º—˜?Y¨W\¾3
?ïö7"¦˜[?g(­p؅?S÷)Ú?g(­p؅?ïùKÑÐÓ?7pJ°ã³˜?JлìQÌ\?7pJ°ã³˜?ïûbÙU¶?=1P¾Rš?BwÁ6Àø?=1P¾Rš?ï×ÒªºÜ¾?xþ ~¾ ?tª¹?î?xþ ~¾ ?ïðy÷àP?lê͔Îþ³?_ïZ?lê͔Îþ³?ïè"*fÇ?XêvKûÇÝ?glÕôYX?XêvKûÇÝAGN4FGL J0151.4-3607?닫†oßüÀR™—_,¶AÀ:Õ,D,À<Â(äû—»@ʆXõµ@ü\Wë‰?Áú"³Ùa?°ÔâšêQ˜?ïœÙŸÄ @ AO€›Ç¿»,€¼}õ#¿Ü|؃9Zë¿é§¢pØ°¿ÚDí$±W¿ê>ku™à¿ïô¸~Œ"
AGNbcu3FGL J0151.0-3609PMN J0151-3605?ïøΖâ–?F¯b€"Œh?OÜÅàîƈ?F¯b€"Œh?ïð9.Ûñ¿?dQ"\9Ÿ†?_¢ z?dQ"\9Ÿ†?ḯ¦'W^?tÓê¦dË?y¿,Éâ4²?tÓê¦dË?ï/?GÚ+$ÐÞ?aÿU~X±?GÚ+$ÐÞ?ï³Ã‹|í´?…ÆÓ$
4?ƒÉ?…ÆÓ$
4?ï˗yj
q?~D؏â*?z4C]ˆ«e?~D؏â*?ï§Íè'ày?‡¬÷
?ê?†…Þ÷}Ã?‡¬÷
?ê?Š;hó?x¯iö¤ô?‰m¶'I?x¯iö¤ôAGN4FGL J0151.7+5455?íþÔq[âÕÀÀJÕÀ:{93'uÀ<)'(±Ïñ@x97Úû@ßçžà*x?Îû"áN?ÎgΛYa?ñ"ÒTÌ
/@ô"µÜÆ?¿¾HyìU(Q¿»äqY3¢ð¿ä&&À^)¿çO[½•ø$¿î,¦AÕÏ?Ø_`'÷–¥AGNbcu7C 0148+5439?ïÝ@1•Æž? <mí¹ï_?q_ç>»™? <mí¹ï_?ïñ}" %1?b;ô6˜úU?]Ú;g—?b;ô6˜úU?ïŸ]÷¾#M?~k¯¾+š?ˆ('w,Ã?~k¯¾+š?ïìA3üܵ?J}—ãoY?c¾ËÎé;Q?J}—ãoY?ïçfœtÈÝ?eÿ0Å@K«?h™c\|rä?eÿ0Å@K«?ï°¡>dÐË?©«o
øø?ƒ×°b¬E4?©«o
øø?íõž·)'8? ÝrË[€?°S
F³vB? ÝrË[€?Ö/Þ?viÜi"n?Œ{
ã¤r?viÜi"nAGN4FGL J0152.2+3714¿ßeÉ»þÒÀ8Sü–ÿÀ:¶ÁȌÌÀ<†xºüÀ°@‡r¨¾û@e%îÇÉ?»üžw?³£çÑ5Z?ñ¯Nìő@ކÀùÚÍ?ïBUåæ¿ãã/áD¿æ³û¢n¿áêP (êZ¿æ:D4w¿ïÏöbreùAGNbcu3FGL J0152.2+3707B2 0149+37?ïþ¥'tìš?{Ÿ`R?%­……ÅÝT?{Ÿ`R?ïõ‰!&kO?Uvëë0E.?Tí½¥jò¸?Uvëë0E.?ïøbˆœ'h?:\oÜ?NuÜÝ}¢¥?:\oÜ?ïö¢`èx$?6­ŽÖ‹2?R»>³·M?6­ŽÖ‹2?ïþ`þø?"¿iñã?)ð,EPô?"¿iñã?ïÙ<å?vJ( »ªn?swaô"QT?vJ( »ªn?ï÷(;čt?`?˜Á·V?Q¯ˆò—£?`?˜Á·V?ïÞhxíw?Z>9Œ>ÃY?pËÄ¥¬:?Z>9Œ>ÃYAGN4FGL J0152.2+2206¿îo[»p6§ÀCM¶¡è´À9²j²üA/À<7Üýœxq@Üωë|@åO±;?¶Y 
ý?¾µ9³*q@+ÞàˇR@[Õ¿É¿³Û÷žBÜÛ¿æOâ+ã	¿èÞÙ	1µ¿ç'Á†¿ïÿùµc#¼?êL»P£‡AGNfsrq3FGL J0151.6+2205PKS 0149+21?ïüýV­`Ì?5äÆ$–?8Li9[?5äÆ$–?ïó&ªR":?a8EŸÿÊ?Y²«ÙK,?a8EŸÿÊ?ïÚî`ñ2?qù^ÐkÏô?rüãu#!?qù^ÐkÏô?ïõÁŒ
%>?C7–…z?T|èKiô?C7–…z?ïûå—Qža?B'i($û'?@i¡½¼·†?B'i($û'?ïÐF6p)‰?Œ ÂCb?wÜä·mº?Œ ÂCb?ﯦŽt¢i?…Ã3ÃgM‹?"\bo­?…Ã3ÃgM‹?ï²d"‡¿…?vg ˆS}?ƒfÚên¶©?vg ˆS}AGN4FGL J0152.6+0147¿i‡X˜UHrÀLÅM@$³>À9mRj0'À<tBÇü@%L=gµ?ÿñ|D=?¯Çˆ"9¿ƒgáfÝ?Ôi,"AC@	B1}Ñ?¬¬j_Lõ/?¸I*ì<ԝ¿ár]ëm¡Ä¿Ü"í*¿à¢¸'¬eN¿ÓVPn­\ÅAGNbll3FGL J0152.6+0148PMN J0152+0146?ïþz?`	?Š´I½Ü©?(\F6tI?Š´I½Ü©?ïõ\)ð›?Y¾Ëϙ'P?UG®AÕ¹	?Y¾Ëϙ'P?ïöÁIÙ4\?V)OC±óê?R}kÏ%©r?V)OC±óê?ïû}×=¶f?1"÷Æ?B¢)f>[?1"÷Æ?ïý.æº?,Ûx*˜?6ˆÎ
Ìêr?,Ûx*˜?ïÕŸj?|'HÚÞ¡?uxÀÄ/J?|'HÚÞ¡?ïõ«â,Á?gìªÙWJ?T¨;lÃoÒ?gìªÙWJ?ïøÉ» U?AOjA^AK?O¬Ù!ÿö?AOjA^AKAGN4FGL J0153.0+7517?Õ-Pèr<*@)É%x_.À9û)=+ÇÀ<L"4­†¶@ TB…Þ?ÿ&ò³c%?·—MŽÿä?±BZÃpÆ?øln¾#¼ž@$ìH`¿èK·ùÖñ¿­Wåš#,¿Öþqàm¨¿à(l/Ô¿à{'{üP¿áÍ´ôhó	AGNbll3FGL J0152.8+75171RXS J015308.4+751756?ïû»ÌŽ'd?3"aÙ?AÎ?;49?3"aÙ?ïàý"5žÀ?pjÙÏÖø¹?ol—‡†?pjÙÏÖø¹?ï塃?oT-ç2kp?j^?oT-ç2kp?ïŠtw˜ŠG?q.éߙŽu?bâþ61?q.éߙŽu?ïð"ÜëuQ?Tçæãâ-«?^öF)^G?Tçæãâ-«?ïe>¦·lò?•Fï''h?"X+,ýÁ?•Fï''h?ïÏ ž¨n–?'îTNéJ?xo°ÁHá?'îTNéJ?íÑiW?—óÞ{ÏBï?±tµBCPË?—óÞ{ÏBïAGN4FGL J0153.4+7114¿ä]+ŠzöI@!ò!ȧ¤À:jfóT À<O$V ž@!"U©€Â?þuêMT?º$ëFàd.¿'y(_ð€†?Ú©=;äó@:šþsì¿ïûÔ¢.=«?ïÿIŒ;F¿è€§?tŠ¿Õrü øH&¿Ü­ÏÜv¸ï¿ß{"¶
nAGNrdg3FGL J0153.4+7114TXS 0149+710?ïþ—ʦ?$^¯"†?.~W3Aš°?$^¯"†?ïîëžÛ3(?cñÖ.!q?aa®ã?cñÖ.!q?ïöÃYö/?D»EJžó?SÐyº ¦?D»EJžó?ïðãrU²å?E÷•~Ÿ=ü?^9ÓÕr?E÷•~Ÿ=ü?ïý±ÂÁlX?+©xm?2që÷/ŒÀ?+©xm?ï¢âˑ¹P?JíJV÷o?‡GM"pãÛ?JíJV÷o?ïö&"Û?aF]cÙ?S³ç6ÿP?aF]cÙ?ï'ƒ%b?qm""iJ3?~¶¾Aëo?qm""iJ3AGN4FGL J0153.5-5107¿Ç"V)¾{ŒÀO¢sÿ¬*À:Ìg¼§»›À<z9ŠeI@üÖ~|\È@
goF	?ô¹©š¿¯"èÁu?áèæ€Äa@øªgr*?ïøs^œm‰¿éú÷k¿éQÃA2Ð7¿îݼ¾â©X¿ïý®aQԉ?ì!1¾iÕAGNfsrqPKS 0152-513?ïþ@YG«?FçÆò ÚÐ?.[ú«JÚk?FçÆò ÚÐ?ïç3ÑqTà?€ûØöH=©?hÌ.'ʨq?€ûØöH=©?îòý¦¼öI?šËâóÓík? Ð%'œæy?šËâóÓík?ïû/vôS?9ì*çQ®ý?CB%ȯÌê?9ì*çQ®ý?ïÿ*¯£h?5 D¹t?ª™Q
Ë?5 D¹t?ï®?…ž\n?'ÏmªÂ$Â?"p'é"o?'ÏmªÂ$Â?ïW(±W®ñ?"šénÑÁj?•éÎ*éå?"šénÑÁj?Sì*$?ŠXÃ"àà?Œ—kõvÿ?ŠXÃ"ààAGN4FGL J0153.9+0823¿êï<ÏÐH"ÀI°·ÃPLIÀ8ðÑn=À;ª¾®&@7ÕÞCl¼?ý%'6¥®{?¬ÐZ¿6?´s"·e•@Jñ£EêÆ@BíPøì¿Ðmâ;sôn¿ÕŽ_©³Ã¿àlâiø¿Õ¥^~~¾¿â1úï,¿éäÞq9þÿAGNbll3FGL J0154.0+0824GB6 J0154+0823?ïþ\ä~ç‰?U†5"þ?*1µ˜5ÙT?U†5"þ?ïò3Ȟ-Â?]3ƒŽ`§?[˜nylìÕ?]3ƒŽ`§?ïìÕvæ?b¾k`??c*‰AåÚ?b¾k`??ïö9‰†?9µÞÕ«6?SÅÌÝód?9µÞÕ«6?ïýHcJR?+2֋üCÑ?5¿†™… ?+2֋üCÑ?ïÎY9',À?y±'ç}B?xÓc;zÆ?y±'ç}B?ïæJ…Æd9?sQ:š"Ÿè?iµz?&Ø?sQ:š"Ÿè?ïá†ÂR'?ZÃS÷j?ny=³³®ë?ZÃS÷jAGN4FGL J0154.3-0236?ïì¾£OŒÀNž¢×/ýÀ:ݤÌӂÉÀ<œ¿eÛüë@| ®vJŠ@É2¼î¥?¼´ßWD5¿©P>Ü´¡?ð¯¢ðZp@Åôw‹§¾?ïíYx0=¿åföyn€ç¿äìÔ	0'¿â!ÛA¯¢Å¿Ö3~݀¤*¿ïÿî,˜å?AGNbcuTXS 0151-028?ïý¹5¸–?#°2<@É>?26Q/?#°2<@É>?ïòtÛ&à?`©ä¨©1ˆ?Zá¿äÎÎ?`©ä¨©1ˆ?ïó¸†Äª¿?að"‰Û¨?XŽòú›€'?að"‰Û¨?ïúµ.öc?.ü̟U?G½+GÿŸ?.ü̟U?ïýZ"ؔ?0?&!ó(?7.ðí¯d?0?&!ó(?ïÏÙ>³m?}·oļ?x`ú%©h?}·oļ?ïõ(Ӏ<ž?b¡x'n…?U®Y
…"'?b¡x'n…?ïã¸àløã?^E¥°?lG¿Ü?^E¥°AGN4FGL J0155.0+4433¿í´Çn$\À0Ú©÷µ®£À:b-—è¿rÀ<C8d@…"†?þ]Ã_eÁ%?Á ¨A'<°?Ós k°R@"¡ô±î@žWˆ
€?ïù$¯ñ¦¿ÓÄÐo½¿ÛÖ}»Áã¿ç2BÝË!Ò¿æ\¤¡	¥p¿Ü9G'RAGNbll3FGL J0154.9+4433GB6 J0154+4433?ï;ùÂhÂ?š)r"fæ?˜€Ç²þçÉ?š)r"fæ?ï¦}ü–OH?Ü4öa-³?†`€ÝÛÉÝ?Ü4öa-³?ëËÌÉ5­P?ª˜¾Ú?ÀÐÌÛ)JÁ?ª˜¾Ú?ïH÷%K?v6C¼uð?–á€~§?v6C¼uð?ìÈÎg£õŠ?¶±©åÿê*?¹¹ŒÂàS¬?¶±©åÿê*?ë5c‰ÖŒ?Åây¸¹ÖŒ?Ã*rØ¥Ò?Åây¸¹ÖŒ?åU™?ÆÏ?µý'ºv5?ÕT́þra?µý'ºv5?ëææ5ÿk[?¢@1¥<ۖ?Àdg(R–?¢@1¥<ۖAGN4FGL J0155.4-0625?ÓÉù?5dÀP`,'À:óÀƒé.,À<–'Jÿ†@r)0zò@>
í(Œç?̇œ–ú?̇DÒ»?÷¾XzëX©?ÿúa÷ì¶?ïþ\AIvl¿Þâ˜[V¿ç·y^:ÈÔ¿í¾I¡ßŽE¿ÕÀŽeˆðÕ¿ïÿ5jE8AGNbcuPMN J0155-0621?ïäO1²¢?™¢qÉDM?k°ë»Ž%?™¢qÉDM?ïàŠŒéæl?ynó2|&?ourïô~?ynó2|&?ïkÐgOß*?‡C׳?8ù?'…ós¶´?‡C׳?8ù?ïàºr'(?XËírzÚ?oEsÙ?XËírzÚ?ï÷ÿÒø0?Q±:ü|| ?P[Ȑ@—?Q±:ü|| ?ïR6ÇÎqy?¢{«÷.?•¹'zè?¢{«÷.?í".1…wè?¥2ì£m2&?³ÞŽrr¿?¥2ì£m2&?îÔþ5®?"ȯÎè›?¢°ÚP)?"ȯÎè›AGN4FGL J0156.1+1502?æÆÈNÁa½ÀF€.#)À;›ªgG6öÀ<Æ´!Û@!w©úå¹Ù?úk³\¹>{?ÕT¤òé?ÊÑ(¼Œ¸¶?ööc3«þ÷@gÙ¦¤ð¿é'æ!1¨ï¿ð?ð¿ÒŠ…¼¿Ü8Ʊ•¿Þϑ7ËHhAGNbcuRX J0156.0+1502?ïý¼¯Ú^í?$ÇÔÞz<?2€¨z¨?$ÇÔÞz<?ïó»¥?Z÷jŽuðc?Y֊*°Á ?Z÷jŽuðc?ïç覿iY?U¸zƟÖ?hYJ5Ž›?U¸zƟÖ?ïö¨.÷~?@ìäÌÿô‰?R¯¢Bå¹?@ìäÌÿô‰?ïþO$¼‰?&Ññ<Ê\?/KT4OÎ?&Ññ<Ê\?ïÍHJûŸ?`qŸ÷w?y[چ¸=?`qŸ÷w?ïêáôlK?i4•Ž1?eƒÕ?i4•Ž1?ïæÄðŠl*?a:ÒÐy*?i;–²?a:ÒÐy*AGN4FGL J0156.5+3914¿É™\]pÀ5èÍJ¡À9ÒU݂&¶À<djQ­q¾@áaKI{@wí"Ó8ø?²jËOõ?šµÉƒŸºÎ?äBÎFIm@…䀝Ÿ8?…Ñ1½¿â'Ÿ¿ùTÀ¿çÿF!!Ä¿åHùn‡Q¿ä_ÞÝpˆÿ¿æyi"ƒb¡AGNbcu3FGL J0156.3+3913MG4 J015630+3913?ïÿ:¦UP??¢ûnõ´?¸±à+ê??¢ûnõ´?ïö§Orì?VÊ4äZªh?R±aš h…?VÊ4äZªh?ïöïÙþIÙ?=¬ñם‡!?R Kê¯Þ?=¬ñם‡!?ïÿKuQï??hèëÌÙØ?'PÐV.u?hèëÌÙØ?ïÿjiˆãG?vQ>õJ?²ÑŸÂqU?vQ>õJ?ïÓ¾Ynu?…:¤Ÿ9Ê/?v ùðÕiK?…:¤Ÿ9Ê/?ïõäòQÓ?XF_Èè¿?T7Ý°(‹?XF_Èè¿?ïþŒW¼ªk?û+L²Ÿî?':'1ïÈ?û+L²ŸîAGN4FGL J0156.6-1758¿íäs˜Ó÷ÀRÓo~=À;NÞÚ‹À<łw>$ÿ@Cl§s!
@EÜ@W?ÅøvHܒ¾¿«—s#¹¹?ã̤ˆàä²@9˜¸=S?ï8ßî°L¿êˆH8}õÏ¿áÊDAxpT¿ÙGőo(­¿â"^~»qܿﱺ!Ï]¡AGNbcuPMN J0156-1800?ïüÉi7s?.¿fÞq£?9´¶JüÐu?.¿fÞq£?ïôe+¨ê?\'ubS™r?W5Ã=z\"?\'ubS™r?ïîb¸†ð?kŠúÏÿY)?aëZ¶àG?kŠúÏÿY)?ïû€Ó¾ÈA?(PÝxq!?Aü°Õ
Òf?(PÝxq!?ïù/Ž/zŽ?Fuã?ê0/?KAƱÐë?Fuã?ê0/?ï˵íQ‹?ƒØ!X"f?z%	yÑRC?ƒØ!X"f?ïì'@Ø?paQïU÷¥?cnìÎF2ã?paQïU÷¥?ïéÓ3#?V«E2£'?f,ùž?-V?V«E2£'AGN4FGL J0156.8-4744?ánšÊ=½ÀPp@ ÇÀ:mDù.T§À<ªfÄZ7"@ŠÃvˆr@Õ~œ¾H?¸´XaÀå8¿›ûÚ'ö7?âa0œýç@	i°|ʬ¿è6úhŠ'¿ãe—=$¿æ
5bhß¿Ý2GZ²~¿Ýw¼Ú¼N¥¿êNHÝêVvAGNbll3FGL J0156.9-47422MASS J01564603-4744174?ïÿŽóg/?øëZr?n&…½GV?øëZr?ï÷­¢:'?R?
=ƒá§?QÞ¥?|±?R?
=ƒá§?ïùLõ›>?\W2)ê}k?JÌ*¸ªÉÊ?\W2)ê}k?ïÿR*;µ/?ÑüÖèR£?º²*Žh?ÑüÖèR£?ïþÏgB´?ȸßQdù?#	‰×¼•&?ȸßQdù?ïÙQ"¦?vŸ1ýá¿9?sswn"ü?vŸ1ýá¿9?ïúøEîÄ?XÄ"7òˆ?Dè9dCÒ?XÄ"7òˆ?ïý¨»†º€?)	õt°Ä?2º"uRÁß?)	õt°ÄAGN4FGL J0156.9-5301?ëqÙX˜¿ÌÀN°å^³À9Ü¡|¼êÀ<³†ª©Œ@¡ 47?øת@°Ê8?´->§…–?º¶¢Êê@F"Ú8+@‰qü­Æ¿ïáâ"Ÿg9?í…ʬk-?¥G´t'Ln¿ÖŠš"U•¿â3EaÞí6¿ÂèÛùe‡AGNbll3FGL J0157.0-53011RXS J015658.6-530208?ïÿBn ­Æ?
û&óž?²%j³X?
û&óž?ï÷)¦ ?U,"N|Gù?Qݬ†ÄÊ\?U,"N|Gù?ïï¯Ð4,Ð?g¡áx•½?`P/¾ÀZ?g¡áx•½?ïýÓ
"ÏA? ZtwÏÑ?1g'½dˆH? ZtwÏÑ?ïÿŒA
ß?‡ÎäaÕ?®zv_ƒ?‡ÎäaÕ?ïÛ£þ¥ô?r›…Xšý?r.uiO® ?r›…Xšý?ï逻ÇÊ?q9²ï¥®?fî$›ÍÊ?q9²ï¥®?ïûíQ&¹'?6ô8òÁŽ?@J»
òoü?6ô8òÁŽAGN4FGL J0156.9+4648¿éua‡ô‡À--"n)ÔÀ:ë<©Ôz@À<h-æÃ@Ÿñ‹¡´?ÿ–îú>¯?Ðy<¬Ù'?՞9¾g¯@Xä1ò@þíï]'?ìç`vã6?ï­Ù¢H>Þ¿Öl|ªöc¿çˆD§Ï½B¿âtÒ9ô¿ðAGNbcuMG4 J015651+4648?ïîÔéž6.?X-t¸OÆt?a+"D1ß?X-t¸OÆt?ïØV¯ÓÜz?Va9>Ý?sÔ¨PÒÈ?Va9>Ý?ïg½6Š^F?…ðÖª6Ãã?"Y0lA?…ðÖª6Ãã?ïoô'ÀÊq?u'ÉL?'{	žÖ?u'ÉL?ïæ )"øg?d/þvn@'?ißÖpÙr?d/þvn@'?ï+9Û(e?¥õÕäzH?š˜Ä–ú+J?¥õÕäzH?î¿ö¯Á›Ž?—Ês0m=î?¤•Uã ?—Ês0m=î?íñ£Ò"ÇY?š ù½Ï6'?°rákaÅ9?š ù½Ï6'AGN4FGL J0157.7-4614¿ì.ç|¯ÀP´˜5‹'À:LvѵÀ<!4x­Ç@ˆW+µæV@ê}ík¨Æ?¿à	ëf?û?ÌꗸîÉw@–l£—I]@A	—ÙP?ïü=¿ÿ	¿Û==ÛWÕ¿åÒ¾^"¿èÛ¾WîÔ¿íþ˜ ó–¿ïÿþR€ÖTAGNfsrq3FGL J0157.9-4615PMN J0157-4614?ïÔªÔÈ?p¬×à¹U?uø*¤fw¾?p¬×à¹U?ïö:—*©w?]¥,˜'?SŠÑµ«Ò8?]¥,˜'?ï&µãD?Œ#BmÏ?›)_lC—|?Œ#BmÏ?ïü¶+ö}ö?&¬Ö-bÖ?:N¢ZºÒc?&¬Ö-bÖ?ïœ+C>‡ê?…Í°¬Ä?ˆõ/"Ÿ•œ?…Í°¬Ä?ïØ3"?uߠСÃâ?sætM²?uߠСÃâ?ìºáñTÊ?¨ÑZC ò?¿"(ðuY°?¨ÑZC ò?ïó­ÄÉH?J¾%Ÿ?X¥Þ`oï¹?J¾%ŸAGN4FGL J0158.5-3932?Õá uù"ãÀQÕQ֌i/À9‰'TPº-À<L~D©}<@îJ µ'-@LQj‹?®p®hß?®¬ˆ×[@Gjdø¨@ÝÍM{2ü?íŽ:‹I¿Ý—Ä{Dš¿áž¾fØ|-¿ãâC çU¿á^û}å3 ¿âaÈýŠYáAGNbll3FGL J0158.6-3931PMN J0158-3932?ïýó"WÏ0?Be$ùù2ü?0cÜLU"
?Be$ùù2ü?ïöXy
O\?X7˜ 1s¡?SOCWH1?X7˜ 1s¡?ïâÐpàË?ya_عU?m/Žéu\?ya_عU?ïý3~Ôéž?#@Mò‰Ï?6d	vbáY?#@Mò‰Ï?ïþz1c>?*Ǭ"LSÈ?/˜Z9€ÇX?*Ǭ"LSÈ?ïÝ7å/ÖC?rjô)Wô%?qd
T×Æ?rjô)Wô%?ïð¨F… h?l×hI?^¯s>ö¾Ã?l×hI?ïúk>×?9¦zf
t?G†Tlˆ?9¦zf
tAGN4FGL J0158.8+0101?±=^O«ÀLÁ¥~ª*À:MŒuĨ;À<W#I±$@.û%OÅ»@d¤Ú¦?µ3>ñ­V濱*óÄa?úõ³;?ï™"/¢&}¿ã·M>w4¿ßêvjG¿éI­=ef6¿âò|Ÿ7é%¿áa¢
×I¿èËRä©bdAGNfsrq3FGL J0158.6+0102GB6 J0158+0101?ï©j ýrÿ?µÍŒu¥»¿?…¥w¶Tl<?µÍŒu¥»¿?ïijcq?°‰ûGo¼b?Ÿ'Òº~iÞ?°‰ûGo¼b?ï6iZPrM?•'gßôX?™2Ô¹aRY?•'gßôX?ïw±{HÜÏ?xÂpü5%í?'	А..?xÂpü5%í?P>0è?˜Üÿè:ä?Z+÷Rýì?˜Üÿè:ä?ç'4´§'?ÐLÄù|r?ÐݗЖ°Ü?ÐLÄù|r?îˆÇw(è? d vN-8?§s†Õ£‰? d vN-8?èp÷ñ¶±?¸ã2O>žÐ?Î< 9'á=?¸ã2O>žÐAGN4FGL J0159.3-4523?è˜WèÒÅhÀPÒt>–=ÅÀ;ûAT^&À<ZÁ#>@ƒ+̱º@ñÀoz?ÃïÊhC‹E¿­Ähœ˜ôÐ?çM}å-@
·y
²ñ?ïÆ­czù›¿ëϚ!~ÕÉ¿ââ΁WÙ[¿æÿ¢!¨qN¿á¬Yûð¿ïÿýç!éAGNbcuPMN J0159-4515?ïÿ>Ò0Â?¸Ñ¶x°?<*<Õ`?¸Ñ¶x°?ï÷¬²%+´?RhiY¸"'?P¦›"¬Y?RhiY¸"'?ïå¥Lïá"?v	Æ
O"Å?jZ³}R?v	Æ
O"Å?ïÿ.*ØH?Æ3[ƺ?:ŸÉ_²?Æ3[ƺ?ïÿ7Xº^ê?…!mÏ9…?ëç?…!mÏ9…?ïßVaX?r(®Ÿæ?pTÏ5ù…?r(®Ÿæ?ïà,…;‹?s6í??oÓzÀUe ?s6í??ïú­ŸyÇ0?;§é<"ßé?EIƒ¹!g?;§é<"ßéAGN4FGL J0159.5+1046¿Ý"ÃM¿réÀHSπÜ3rÀ99I—"ÇÀ;ù'ì®@¹O"ðB?ÿa,:=é?­ÊÞW†? ¥ ÛN½?ó(᠙h@Aàz~¡F¿ÝèÀž@Gn¿Ý/ò6ᄿà†=~搿áüŽ''Û¿Úª-e"؏¿ÛLáD¨ücAGNbll3FGL J0159.4+1046RX J0159.5+1047?ïþԁw
þ?U«5_ø?"·ëÈÄ?U«5_ø?ïóÜÇj­?\H#Æ0ãç?XFrG¥©?\H#Æ0ãç?ïö·JF=?U¾ûF"}m?R'k‰þ&z?U¾ûF"}m?ïýG:?$Y|Å ]?5ǐïj^?$Y|Å ]?ïþòÐcý?$(þt…sJ?/°Ô9À•?$(þt…sJ?ïÎîe"ïn?''ܔÇ?xˆÍTkA	?''ܔÇ?ïõ­Eç"?fUN¢5°¢?T¥vHf8?fUN¢5°¢?ïù×u$ø»?>7§»?H¢+k˜¥?>7§»AGN4FGL J0159.7-2740?áÌÔã¹pÀRµ;Ÿ_À:"z-ëÀ<ÍÄC'O@È÷C«@
¨_/:€?·iŸUñ#?±]CRAf?÷Ê	ÞÒ@È7Zµ-I?ï÷"_mλ¿Ú]&š¯™¿àÁÞây|¿àÂÞZ"Ê¿ââ½ÏÚ¿æÑT¼÷"AGNbll3FGL J0159.8-2741PMN J0159-2739?ïü–rÒ?/H".ÄE§?;OBY«ã?/H".ÄE§?ïô¶ã´ù?Xˆ?¥ï€?WΒ–là?Xˆ?¥ï€?ïï÷¾àGu?l›Ð¹•X?`A?Tò}?l›Ð¹•X?ïðr96
1?Fõ"YŸQ?_ŽœMÓ?Fõ"YŸQ?ïù0xÌM)?A"«éFt?K>-·G¸?A"«éFt?ïÖóVÏD¡?wt,6d¢?t†T³*£8?wt,6d¢?ïß}ÚSüŠ?}

ÉFU[?pAçß²ä?}

ÉFU[?ïÒ¬X@¼f?d*Ãß#¢®?v©ÓÏӘë?d*Ãß#¢®AGN4FGL J0200.3-4109¿Í3\è}MÀQ"Ó0"'À:‡4–àµÀ<'oQÇrñ@ p6åDgä?úéQgÑ q?ÁblÇ(ž?Áۛǜ6W@)ý¢W®=?õA÷˜(«¿ïÌ7Z?åéáæ9…]?£ûüÞпښr¦æ‰¿ßGH~sùL¿âÒ*AGNbll3FGL J0200.3-41081RXS J020021.0-410936?ïücî'î?8Ïú™=T¹?<à‹dsʧ?8Ïú™=T¹?ïÄýq–?cùÅ@uî?}þ_B%?cùÅ@uî?ïØÇ<Xæ?xºEj'œ?s÷œoõ
?xºEj'œ?ïuq†#+?u´Æüí;®?'QßÔcŒ?u´Æüí;®?ïßF0)Ø/?n½û€ðÒz?p\çÊǔu?n½û€ðÒz?ït'o/¹?¥èr¶ÿü'?ž'{‰¤æ?¥èr¶ÿü'?ï¨ÂÙ{SU?‡ººNæ…?…ÏI¨
b¿?‡ººNæ…?í^Kž?¢§B95€À?µ
§?kó?¢§B95€ÀAGN4FGL J0200.6-6637¿í¥Mܤ'´ÀHŠÎóÀ:#8ê,YÀ<…6žË2@@zž×œ	@ÐeÁ•?³î`¬ßX?'dmÆ_¨æ?ÙiôE6ÀÜ@pXËô
¿ám‹zÖ¿ä'z¡†Î¿çúVÞ3&ž¿äUûŸž¿é±Èd¿ïú3¢Ä»†AGNfsrq3FGL J0200.9-6635PMN J0201-6638?ïþ¼°ž?ôÎh
}?.ä<ê€N?ôÎh
}?ï÷d_kÙ?RKÈÞ¶?Q7A Ή?RKÈÞ¶?ïìÎí‹?O2å²É/?c1îè"^?O2å²É/?ïÿ4þ[Ýn?	rՂÙ6Ž?`9Î
C¡?	rՂÙ6Ž?ïýóŸ/ÁË?%f<…Š?0c'""?%f<…Š?ï؅à¶?'©ƒ!(2ë?s½v«s"ß?'©ƒ!(2ë?ïépCVc[?h%KíRú?f¼áö<K?h%KíRú?ïý¼[#?'-"‰Þ?2'ý¿1=?'-"‰ÞAGN4FGL J0201.1+0036?ïr݊+´ÜÀLÌڐî¢À;~eæä¦À<ÆCnÙÒ@!4՞'?ý4¥ùú-?Ñ"×ü?®-žÁ0?ßŐÃ\5¶@‹ìé͹‡¿ïL³'#i?ít來
 ?ÞF}¯y¿Øá<O¼¿Ýü"C¿‹¿àqS>ìNóAGNbllMS 0158.5+0019?ïÿ+>!+?É%q¦?ŸÞǂmÄ?É%q¦?ïóóyE"?^³•,ó?YàT휖?^³•,ó?ïóšŽX•:?Ed/ñ‡†º?XÊãF–|V?Ed/ñ‡†º?ïøêÒ=ÇX?5)d%–áº?LTµý´3º?5)d%–áº?ïÿ$Y6ä)?ü2C¤át?tà7y¤ö?ü2C¤át?ïÕXþZÁ?vL!ú¥Dí?uS€Ùëª?vL!ú¥Dí?ï÷¡–W¿?UðxšB?P¼ÓZ-'"?UðxšB?ïîêí&çÿ?SÛëªÞ½r?a°¨Æ?SÛëªÞ½rAGN4FGL J0201.1-4347¿î—šë)ÀQóà7ÝÀ;­†)zLÍÀ<ïÈN¸Ê·@!ñҕ¹?úÞ@'—?ÑV€[¯ÿ?ÇZHJòlš?÷žçf¬"@4•¥RÝ?âÖtì;'?ÎR	!¼¾7?åǂ«@‹¿ãæxw¿¥™ÑÞë™}¿å²?'ÌÎAGNbcuGALEXASC J020110.83-434654.8?ïüå÷@=Þ?/£¦áŒD?8ÐGå&| ?/£¦áŒD?ïô×ɼ2\?\¦Khê^?VPlBãW?\¦Khê^?ïÞvæð?q#À®UŠ?põñ6Î2?q#À®UŠ?ïû·ç"
?1à¦^œZ?A ce;¬F?1à¦^œZ?ïù‹³Á§Ä?CÊw÷j€?IÑ0¢"hX?CÊw÷j€?ïÛòÔK?sÛbB¾Œ?r•Ú>Ç?sÛbB¾Œ?﹃¶G>?'"ÕëÍú?Ÿl µ?'"ÕëÍú?ïõ+újûÞ?P¨?z¼Ñ?U¨t?Ôj?P¨?z¼ÑAGN4FGL J0202.4+0849?ïvOÖ4³ÀI0ߛÜjÀ:Ðè¨ËeÄÀ<tíSUª@ õ.vŠö¿?ú'4Û©ß?ËÏö¸X¡'?̸Ž;íkÿ@H&	@Êúmnî?é¥C†g®¿êâàíB¿º¤›?áíE¿Êü¬äOx¿Þ1¯$›?â¿çJ¼¤¡5AGNfsrq3FGL J0202.3+0851TXS 0159+085?ïýNÉ"œ?&kC'9Ï?5‰µ~s‡'?&kC'9Ï?ïðüÐSG®?[Ü°h¿¼V?^_"* ?[Ü°h¿¼V?ïê$ó̸?g¥³ÐžàÎ?eóÛ
Óo¶?g¥³ÐžàÎ?ïêC>)lœ?Jám«Ïbñ?e¼Áèq[Ë?Jám«Ïbñ?ïý
˜=Å?5}…¶xJ?7«>ÌK½p?5}…¶xJ?ïÈö·Ï1?ˆ4{Œ…?{ðÀõG?ˆ4{Œ…?ïäAI»#Ç?u¬×¦§ï}?k¾¶A?u¬×¦§ï}?ï·˜˜'³?q|ŒaJd?':™èI¯?q|ŒaJdAGN4FGL J0202.6-0258¿áâïÅ0‡nÀN9a€M˜9À:sëLÔÉÀ<cݯs²@7súž@óI¾ó(?¿L͹ð…?œÒ¡^E@ã?ÜðqA¶®¨@À¿aKæ?ïóÒà¿ç1e}³4¿ä͇§ÿê¿Þ¹%˜b¿ïÿÍ?¹Ss?ïøŸƒ¾fAGNfsrqWISE J020239.94-030207.9?ïí¡Ä"öË?`G«Ç5âz?b^;¯aŒ¢?`G«Ç5âz?ïòÏÛA?bTÁoÃÔ£?[ÿüvFüé?bTÁoÃÔ£?ï¶Ç§M¦?|,¡ °ƒ?'N>˜<Zx?|,¡ °ƒ?ïòù|u?F²ú>â²Ý?Z
Ŋî?F²ú>â²Ý?ï­x@®pì?€›F]ý?"¡ïÛBüí?€›F]ý?ïÉéØ÷'"?€î!!s§?{o΍û?€î!!s§?ï«@VÿŽ?ˆLï³0ãZ?…<oí¯¸˜?ˆLï³0ãZ?ï»IJnt?rä¸m'?>ŽÓ¼Xø?rä¸m'AGN4FGL J0202.7+4204?År"‰d9³À2ÞD""N×À:¿í½qæÀ<ŠÊ'_éu@ŸøUӍ@ª‰žyÓ+?ÅJ¢Ô€Ë?·ßT"@X?òΝ‡dä@M>ê¡t¿éæÓ^6l#?îß¦Ä$ˆ¿ædèÕ.›¿ØÚf}ãZ®¿å¨Ñl×Å¿ïþÖj€˜AGNbll3FGL J0202.5+4206B3 0159+418?ïÿ3£Ü°?ÇÉQ"lO?‹œå6	?ÇÉQ"lO?ïöZ±¹?Sø6Š';?SJž0Ł<?Sø6Š';?ïõ8Kuõ?V*ªèêAT?UՏ=ô?V*ªèêAT?ïûJ‰;'ž?'w%­ÕOg?BÕÛkäC?'w%­ÕOg?ïÿT<©dÏ?
xÍ.ˆ¬?xmFuI?
xÍ.ˆ¬?ïÖ¸,›ƒC?d"Ev?t£éª¯:É?d"Ev?ïöKAZ?`'®©°Aï?SÓi•	,ö?`'®©°Aï?ïñD<‰·é?O:ƒa±dS?]w†§×þb?O:ƒa±dSAGN4FGL J0202.9-0225¿ì/¾µ)dÀM÷Õ<ÝÖàÀ:Ó¡ÏɏÀ<|%ä–.@ ÈAÒt>?þŒÇÄOOÉ?ÄÊàä[ߥ?AB g"×?þp'Ldë¿ïïê^-1ç?ïá¢!¨¿à:r•;¿Û907Ö0#¿ê—Š@
\$?ÙTÎäT'õAGNbcu3FGL J0203.1-0227RX J0202.9-0223?ïùÆ%Ïك?mX·L>?HçhÑ®?mX·L>?ïðúéb&2?`Œ þ³êË?^
-x,»6?`Œ þ³êË?ïÅCmµ\?xmóTÌ72?}^I;O7Ô?xmóTÌ72?ïìýÆÀ?PJ¦6PÌæ?cåúy?PJ¦6PÌæ?ïñ·N¨
?Y¬ˆ}ø1_?\'cD¾åõ?Y¬ˆ}ø1_?ïËç–ôðû?|eÂoL¦?z4¡b‰?|eÂoL¦?ï'öׯ¡:?Ú°´?©?‹'J‡Mj?Ú°´?©?ï¯Ç¿>;?{€ðúiî?":
Ë3?{€ðúiîAGN4FGL J0203.6+7233¿ìÈ@">Á@$ä$=Ìê)À9ÛtÄÍúÊÀ;Ü|©žÊ[@iŠ·( ³@@Tƒæ?½Û"zÿ$¹?¬`áZàK?ðô:æ…Û@0aV݁?íh"ÿ‰;¿ØŒö=^…F¿ã¸j¤ ¿ã¼]ž–®ƒ¿á…òB}(¿èRçcQ0AGNbll3FGL J0204.0+7234S5 0159+723?ïý¥CB±?"›sÅC¦.?2ÕçÿÏ»#?"›sÅC¦.?ïò8æÉH?_3ÄæÁðò?[Ž3ö+ß»?_3ÄæÁðò?ïíd˗ԯ?n(j ¿ñþ?b›4'Æy?n(j ¿ñþ?ïòÕG—?@±TÀ
­?[ÂU:bµ?@±TÀ
­?ïøâd/Œ?CŽB'µ¾¥?Lvo"ØŒ–?CŽB'µ¾¥?ï³.Ÿ¿gM?
ñ2£9'?ƒ4X"ˆ•?
ñ2£9'?ïÓ¿%«qo?"bR–?v m	xÑ?"bR–?ïξ¯R¾i?dµ¼¹?x ¨7c¾?dµ¼¹AGN4FGL J0203.7+3042¿êòPW0h~À=£gŽÀ8—'¡}"À;°-,ˆõ@z<c3@ )»»,'?£N O´Q?¹9@}ôwŒ@¹Wɱ@š³ÿʥ¹ãf_¿Ý¶µÅIK¿ã½ÊÁ.Þæ¿ââ!LÖÈ¿éy"ù÷¨¿è²#3
ïGAGNbll3FGL J0203.6+3043NVSS J020344+304238?ïùÃo£Hf?Cdwà¿ú?Hò@à¢:H?Cdwà¿ú?ïð–Îì•H?g^xlÓ?^ÒbXÊ?g^xlÓ?ïÚ¶®8ž=?s
œßå?r¤¨÷ž;?s
œßå?ïÿ=å`8ò?	ö^»‹u?CR½†¾?	ö^»‹u?ïõüØm?MMc®2Á?Tî²·å?MMc®2Á?ïÈÚFTo?‰²‹'!­?{'ÜÇYÛê?‰²‹'!­?ïh(†??'ßFÒnÏ?'úÿ?8$?'ßFÒnÏ?ïþâB)ñ?'	$G	?/¡ÚB)J'?'	$G	AGN4FGL J0204.0-3334?â-}5N°+ÀREQ.ƼèÀ;1ºÌð;À<Ïïå։@ ŽÙw*.?û­ L;Aõ?Ó5šìð{?Á61u?ðßn	È֞@Œ_Ó¥."?ïK°¢ÊšÃ¿é÷3þŠ4!¿×c.qÊH¿Öž*¢ëÒÌ¿à$>adŸ¿èý?[_¢AGNbll1RXS J020413.6-333345?ïÿ$rr…¦?
þ,\nŠF?qª 'MY?
þ,\nŠF?ïõQ\­Ä¹?Uˆ2_ú$?U]F§6>Æ?Uˆ2_ú$?ïî¿GA÷¶?ufhñ"\ß?a@¸'
JJ?ufhñ"\ß?ïûÃy€¹=?&6@9âƒk?@ò‰×Ù?&6@9âƒk?ïÿø³¹?'!Éýp? ï
À0?'!Éýp?ïÑé
p$?{‡a`	ƒ?wzïIÎO?{‡a`	ƒ?ïóúú˜É ?qˆš¤v¹?X

]ºð?qˆš¤v¹?ïôÉ¥U]?F"‹5
?Vlµ3HÄÏ?F"‹5
AGN4FGL J0204.1-2919?Öð[å%€ÀRuæFñVÀ;«*ÏÀÀ<÷P²ŸúÝ@¾žÆ)D?ôÎ3Ÿi½3?âUÝLvÑ?èõ €"Ž@V–8@[ul=ÀÖ¿ÒÞÎWˆ?åõ•äsx¿B­­ê‰v¿Ô1‰$i¢¿ç©$@üõ_¿ïü5ĊßAGNbcuPMN J0204-2923?ïù ë¦=?EGh-‡?I´aå+ø?EGh-‡?ïð"lÍ"?`}Àõ¦ÿ>?^÷Ïi|í?`}Àõ¦ÿ>?ï¨Çè?{",—Zt?…Î8Rnò-?{",—Zt?ïÕ.Ó?_'{Š?u³ëu?_'{Š?ïð©"?[ªàër[?^­Ëxæ{?[ªàër[?ïÅ¥uŸX?`gZQ¨?}-}ßM[¿?`gZQ¨?ï|…z[nn?ÁN>|g…?oP´'26?ÁN>|g…?ï©Zœ®¡é?|á©/¾$?…©XÔW…£?|á©/¾$AGN4FGL J0204.3-3140?æIfÑEWxÀRa	éÍ³À;nÈÏJ«À<á4s¥J@&ky˞@d‰Ø[?ÈÐæ¿'æÜjl?ÊîVŠPPz@˽€~•‡¿èòÁS¿ØÔ¹*X™¿å!s¸^€¿¿ä´_î}!¿Îüâ~ºÆ¿å2R˜SH|AGNbcuMRSS 414-035156?ïþQH`Û§?I$D²»?*ëyyST?I$D²»?ïõs?UÅ?Y.¶Åye?UÏቅ@?Y.¶Åye?ïê?XÐ\Ìy2Î?aXG´†'?XÐ\Ìy2Î?ïþÔ!]{d?¯V¨?"½îÙ=0?¯V¨?ïýl²…η?-ƒ,aP}?4šlû'Å?-ƒ,aP}?ïÑÜo×ÿ?'©""íìç?ws'ÒbÔZ?'©""íìç?ïïŒh¿Ã5?i%;çœ?`s—{V~?i%;çœ?ïøy]†eW?E''Ðw«?N‰Ø¬5?E''Ðw«AGN4FGL J0204.3+2417?à{YïrÀAÔdE#öÀ;8é
55À<¦²ò03¤@ ãóÏ/?ù)p;Ò>&?×µZÀ?ö?Ô
ª]·U?ÿ"!bPW@®A·/£?ïÎ3i¹×þ¿ÒÙxÛ^¿æ†00Is翶Ҫ¡¬¿Ñ¢#ᆘ5¿ïÿ® A§AGNbll3FGL J0204.2+2420B2 0201+24?ïþ@o©(?%
~áAM?.Kø=Q«?%
~áAM?ïóÕß½aÂ?X†ò½Â+Ö?XT@ˆ%?X†ò½Â+Ö?ïÚzÒÚ?oÎ~ª ?r–w'å?oÎ~ª ?ïúÅïkÐ?2fӝs?DèALšp+?2fӝs?ïÿkÓ¥?7ˆáÎvß?Áiµ¶?7ˆáÎvß?ïÒ²,7–o?w¾¸Me?v¦éÎç4|?w¾¸Me?ï傣ˆÛ±?r›‹_Ú?j}\tdžÃ?r›‹_Ú?ïðQ(^w?SÊ5tD?_]¯QŸ{?SÊ5tDAGN4FGL J0204.8+1513¿î¯ºç¶ÌÊÀFŸÂ¨†œÀ9Q/¯ðóôÀ<0rÅð9¹@Œe¨%x‹@ª?Ú
£?­ÚÉ呿±?µ=+Y m@ä¢üïªG@ûû˒æ?~Ãvˆr€¿ä"¢A]îH¿ã(Ÿ[zz¿är_îÓ¿êl5恿ïüÑaÜéÐAGNbcu3FGL J0205.0+15104C +15.05?ïü¢
‰é?6Èð¶Ý¢Ð?:ï° ú?6Èð¶Ý¢Ð?ïõ‰ƒï/Æ?Udá¶PÏõ?Tìø|V$h?Udá¶PÏõ?ïãŠnáè›?kí*üTã?lu'GR´_?kí*üTã?ïü'×ÕáÁ?+Z,šv×?;i?ÏBE?+Z,šv×?ïûuÔîYd?8ÑLʵ"?B(¬:'4¢?8ÑLʵ"?ïÓ¨*ó¶?xpÉ!4í?v+ëS¸ó?xpÉ!4í?ï²	!¼¾7?…—U¤[Æ?ƒ}·œ9?…—U¤[Æ?ïøM‡Oô?A[ìZ*?OžÉãLîˆ?A[ìZ*AGN4FGL J0205.0-1700¿éêwwÛ®½ÀQŒí"1{À8ôh§‰FeÀ<DÕòæ<@Ò}'Þ[@ƒ&ùz«?¨x'¼›?´ç<t$•@XxœÉÏÂ@Ôo{bø¿×¬| 9›Ø¿ä¸MžïCð¿èpžmhä¿éŠÃæ¿ïýò߆õ¿ì"ñÉÜW"AGNfsrq3FGL J0205.2-1700PKS 0202-17?ïþ)ĨÁ?&vŠmÚëP?-c·¯4-«?&vŠmÚëP?ïôÕ!©?az3˜uç•?WðUÔüþº?az3˜uç•?ïÚ&øšä{?rtXI²Ú?rìƒÒÚZ?rtXI²Ú?ïþϏ†œ?ËÖvš?#ÛàaI?ËÖvš?ïþïwz='? @FÞ¿Ó?!…'ꔟ? @FÞ¿Ó?ïÌöbiÎó?"$?=Kž?y"ÎÌx^w?"$?=Kž?ïØ×-?uȸï÷Ù?s"z{¿9¡?uȸï÷Ù?ïü¥h7|?;Ò[ð•?:Ô¿ùŸ,w?;Ò[ð•AGN4FGL J0205.2+3212¿çÍûÃQÆÀ<†Â&€À9#T˜Þ‰À<
qÉp÷º@\b}x¦°@kÛñ,þ?«°
ÏK'?²)­ß‡ö•@S¤!²Ø/@<¥Á›p¿ÊuIRk¿åò•ž¸<r¿èTS¿DÎç¿èQ°''¾¿ì1Û¿ÙÊ6¿ácA&
AGNfsrq3FGL J0204.8+3212B2 0202+31?ïþx£LBE?¾œ³w¯é?(uÊд?¾œ³w¯é?ïöY&ü‡ê?T³¾GÊ?SM²`ŠÚ?T³¾GÊ?ïäkM?pÍyÚßL"?kçᓔÛ?pÍyÚßL"?ïÿ<ôے@?DiÐÁ˜ ?ah5Ÿ}Ø?DiÐÁ˜ ?ïÿ/sWˆ?ÍÛ'Ø#?Ú
ß L?ÍÛ'Ø#?ïÔ"z	?"@gxe?uîÃ
y™Ù?"@gxe?ïá,Žº~¨?pbø¶…¯?nÓqc½è?pbø¶…¯?ïþÐQLà?#äO$|%8?.Bûú?#äO$|%8AGN4FGL J0206.0-0958¿êzáV,î‡ÀP[2 f<uÀ;ˆv{‡_ÛÀ<ÊXÓÖ¬@!Tÿ™Ó¦0?üámÙ!næ?Ðrñd0×
?•ñ{ؾr—?Çn,ÙQëZ@%v\'É¿áî=•ŒÄŸ¿ìäÚEÀ¿Û̘ÊfÀÿ¿¸4ûï¯P¿ãŒÛE5"7¿à!4-.6tAGNfsrq2MASS J02061590-0957174?ïÿep°®?1qz%ú?Qÿ'ÓÅ?1qz%ú?ïô£2?X ÔP?V¹›~‹u8?X ÔP?ïøbŒ^•?`ûª³A?NuÍÖÙmç?`ûª³A?ïþߗæÍ:?
ñ̲ð¼˜?"~ÅÔ?
ñ̲ð¼˜?ïÿ³Œÿi>ûJDÄOJ?¬H܍¶>ûJDÄOJ?ïÚRø±"G?tÄÊA¦—E?rփ¿C ‰?tÄÊA¦—E?ïûµÖÄ¥ê?UÈÒ*/+?A(¥½7¤?UÈÒ*/+?ïüb2‡Î?4¢?
¥?<ïEÚ'®?4¢?
¥AGN4FGL J0206.4-1151?îiàS'NLÀP­[[ÕÀ8üQo^]À<(.Ï÷#¸@mO–U¨@TdÏ?¥
¸À¦N?¦'ÎI#µg?ýUúX R†@P+ÁÏâ¿Ò×Gd˜…ó¿ãlh'î¿åÞûmÊö¿ãPPzkÖé¿é={Uá³å¿ïÿ3òuÓÂAGNfsrq3FGL J0206.4-1150PMN J0206-1150?ïþ%žu?>Ð.…ì??/
£…ZÕ¢?>Ð.…ì??ïôo	Dš?^*
å"ËJ?WÍ"4î¬>?^*
å"ËJ?ïæO^{Ð?rqÚVƒàl?i°¡µª@æ?rqÚVƒàl?ïÿu¥\Ž?
MÅXý?KJ͂ø?
MÅXý?ïý×Ê_gÍ?(/usuÁç?1A«•3S?(/usuÁç?ïÔHî É?€–AƐ˜?uÛðޗU?€–AƐ˜?ïÕµ³DP?€O—9ê?u%&>ÓÜS?€O—9ê?ïÿ.71*Ö?Vˆ°Ä‡y?9â\6?Vˆ°Ä‡yAGN4FGL J0206.8-5744¿ÖOF¥¼ù¬ÀLP64êÀ:ÌÁTɅðÀ<ÅZã{dû@·´Œº?ülA÷ò…?Í7xý—ÅÚ?ÆæÇ	i`A?úÀÇ¯;@ÿ¥' T?ïÿüÚ±'Þ¿êM"M1â¿ÖKž¤pb>¿Û¥i±t'¿àé"89,q¿ê"]u&ÊAGNbcuSUMSS J020640-574948?ïþ¿æ+åÙ?+ÑR<õq?$ ¡Ù¿@?+ÑR<õq?ïöcÁñQ'?Sî'‹?S8{Õäý‰?Sî'‹?ïèám˜´Â?oå¾ÀÚx?g'¡­q?oå¾ÀÚx?ïú´¤aô'?,G÷õ…êS?E-n.õ?,G÷õ…êS?ïÿ\?@cõã?=³t«µ?@cõã?ïڑBKî°?€‡
é‹>?r·^½ÛÜJ?€‡
é‹>?ïÝN{I]¨?utŠÈ£À?qXÂg¯ÃÓ?utŠÈ£À?ïóŒí8Ó?G⿇ÿ»$?Xæ%èV?G⿇ÿ»$AGN4FGL J0207.4-3855¿ïê†;mê>ÀQòº`À: r̦6`À<´zˆ\Zt@5ôå?_@Œ|½ÀÀO?¼J^¼?¾g:vÉ`?ôšøÄ¢[à?üòUû_1i¿äÐG«<#¿ÛnÂÊ £¿åÇ]Œ£¿ëÒ ;I?fßހ(A¿ïÿõ¹U ÄAGNbcu3FGL J0207.9-3846PKS 0205-391?ïûà ;´·?>è'sDç?@€ Áuµ?>è'sDç?ïïÙ֏]?e­9™´³…?`&)~aVs?e­9™´³…?ïÁÍÆ$š?xRØ=cû·?	ß}ƒ?xRØ=cû·?ïúŽÇXš?7¸ž&"&ç?G™Åb(²l?7¸ž&"&ç?ï×u#\jS?x«á§{¸?tEn`éq?x«á§{¸?ﲎ,Õ?'ç{"Ž£?ƒ\}	c&¦?'ç{"Ž£?ï"KåÃ?—"×X_ö?œÜ¯q[Ý­?—"×X_ö?ïÄ
êÐÕ?v­"AG?}úŠˆ;ò?v­"AGAGN4FGL J0207.5-1049¿ºˆˆ@®=ÀPr½f'|À;^ìz>À<—6>@!¯vz° @êE%£þw?ɲN¨Ú¿ƒdZ¦gr?¼ 
|xˆ@ã9ÇÝû¿å™‹¢
+}?îñŸoÇc¿é‰Êï|û¿íJU^×&?ã_Nyà–®¿ïúÛ2ÁlAGNbcuPMN J0207-1047?ïƒÔõ (?·q#gÒæÜ?
»KÒ?·q#gÒæÜ?ïó³€lï9?a°/-x2?X˜þÛéþg?a°/-x2?ïÃöëÀi"?I~Dš¶ë?~Š	Íîê?I~Dš¶ë?ïÿʋ)u>ô´V¾ïŽî>úºXšùïª>ô´V¾ïŽî?ïõ]-òEq?YniÑ
Ã?UE£Æ>ÎR?YniÑ
Ã?ïÐï +;?||¬ÂÎî¦?wˆoÒU4Ö?||¬ÂÎî¦?ïŸÞØO?ŠÝšFÝ?ˆ=ÈxÚPQ?ŠÝšFÝ?ïþD(T?/.—e ×Z?+¾jŸ)um?/.—e ×ZAGN4FGL J0207.5-2402?î®î·Ð‰ÀR$œM©?À:F´ -œñÀ<•S–€	¦@̓P:@FúZ¤'D?·¦53h2?Dd!×Z?ã€e`WÆ@*'Bðë?ìpÐL´
¹¿ÞJp¼€¤U¿âŒ
¿Ü$¿æC$Aþ¨¿Ô³œzª¿ðAGNbcuNVSS J020733-240202?ïþ@¾E\?#Úºa•e:?+ôÀӃ™?#Úºa•e:?ïö'¾e'?TÀ-¬´r?RÝæÁü~?TÀ-¬´r?ïïˆÉ'°œ?eÃ3¡»!º?`w6kï‹Â?eÃ3¡»!º?ïÿvYðٔ?' ?E/?4ÆÉÎgë?' ?E/?ïý0•4É?0øÈzÄ?6{V"éU¼?0øÈzÄ?ïÖp§)q‹?€¼ôf;—´?tǬ†Äp?€¼ôf;—´?ïíH‡s?oòŠAO9?bë¸UE2?oòŠAO9?ïÿ
ÙðN?`"¶ã¹?¤Äîvâ?`"¶ã¹AGN4FGL J0207.9+2203?ã²*
PÍÀB¹v_Ø­¬À:ýîðäJÀ<‰iêe;@AhÃbì@5ëÄߘ?ÊθŠJœ0?ÊRøJ~ÿ:@
Vz`o?ÿ2]šåÉô?ÔÚ³àl¼Â¿ÔÜõ8ü¡¿Ëe*§µ¿étËNG‹°¿ÌiýIÂ@Ø¿ïÿ€éŸkkAGNbcuNVSS J020801+220241?ïõ"IÀµµ?M+bDÈÐÍ?TÙlœÑ&?M+bDÈÐÍ?ïçml6i?oEÉçØÕc?h'"¾×M?oEÉçØÕc?ï·«?£?z²Oá¨F?'?•@•X¯?z²Oá¨F?ïÍüA{í¯?`$VÅ3NU?yß6Z|È?`$VÅ3NU?ïëŽnmEÿ?_q0nî?dq'§W©Q?_q0nî?ïyŸF׫?"ÿtŸ!3{?ßŒ%
¦?"ÿtŸ!3{?ﯽrfÐ?•:¾"ïð<?ªVڐ?•:¾"ïð<?î®ÔßôO?"´hÞØìT?¥¯m?"´hÞØìTAGN4FGL J0207.9+0953?Ê!ÚóMŒrÀHL	¢@1HÀ;U&£øÀ<a"ÌÐþ‹@ƒÌ_"?ü³^f½¤?Ü~9¡ŒW<?ïû¤$èî@›Ç;"T@¢°çiR?ÒËA&»×¿Ó"2ëƍ¿Ø{{vmð¿è  ‰wãf¿é¸âό¿ïüÒÿ@èSAGNbcuGALEXASC J020754.55+095014.0?ïòžё?_Èë
¤F?[ðÃÔÚþ?_Èë
¤F?ïÔÍò30&?z'¡"†?u™á˜yE?z'¡"†?îØ,ºG¹?'‹žÛØq?¢}4]Oi?'‹žÛØq?¡'É?î°…"?¥–eñA8i?î°…"?ï{@K°¾µ?'÷åŽÁw¥?—öÇaI?'÷åŽÁw¥?ïbÀa©?š~÷U,Df?"§øòIÓ?š~÷U,Df?ìw5z‹2?¦¬²ÏD?¼FT/#¦p?¦¬²ÏD?ë9/éq?°aZú&Á?ÃC÷ÀZ<?°aZú&ÁAGN4FGL J0208.3-6838¿é¯@4x'žÀGyÂôÀ:oî'B³À<£ˆÁÛC@F¶š[`y@uIÞpc??¶ØrGp,¿£=Fÿ».?îó^ÂC|@¼3Æ«öh?ï0hå¿¿æNèÑQ­¿ç|>¿ÙI]¿äÁgÿBÀÅ¿Í
­B˜ÖÑ¿èÿ[_¢'AGNbll3FGL J0208.0-6838PKS 0206-688?ïþxA–^?™n{õÉÅ?({ã_B?™n{õÉÅ?ï÷АÉé?Pf"ÂðÚ?P^ÞÕØå?Pf"ÂðÚ?ï÷"}˜¡?Zñs´Ógä?QºÅI†í×?Zñs´Ógä?ïþP¥´Úé?2P Ã-J?*õ¡ aÍ?2P Ã-J?ïý¤ŸËє?'›ÛϲM?2Û›9ݔ?'›ÛϲM?ïá‡þÖN?pºƒ]
ëZ?nxhêµû?pºƒ]
ëZ?ïø+	2%?^kçy?OQŒ
Tf?^kçy?ïøkÈ¿»±?B‡ŒŽû·?NPÝÎk´?B‡ŒŽû·AGN4FGL J0208.5-0046¿á¦oÎ͋—ÀLæ…3±tÀ:™ôàèÄÀ<Ã¥Üû@œ=n€@§¬Y¾O?ÀD
Ý)¿~ÀŽ–—m?Á™ÁÕ?þ¶E|â¿ãÑx=Sr™¿âDr@bï¿ål"ABÀ¿Ú5…=A)¿ì4"|+ʉ¿ïÿý±q&´AGNbllPKS 0205-010?ïé7…8ŸÀ?j6~Å?~2?fÈz¥(P?j6~Å?~2?ïð‡Ðæ¯?i[úzû‹á?_òð­4?i[úzû‹á?ï¥cÁ'ÔP?…3uÉòÅ?†§Œ|?…3uÉòÅ?ïêBÙÄW?O:‡£O?e½&³?O:‡£O?ï¿âò0½?v
¶vôþð?€Cf»?v
¶vôþð?ïÌ.A~G?z>ϟõ?yóèþ-XX?z>ϟõ?ï·í‹ÅW?…wAÉÜ©û?'>Ĩ
j??…wAÉÜ©û?ï•Êð²7Ô?z
ëÓ7žø?ŠCá0{?z
ëÓ7žøAGN4FGL J0208.6+3523¿ÙÙ©‡µÀ8ÞT´:çÀ:¢zˆ\ZtÀ<|î¡2ë@ ¬í†««??üä17°pv?Ãìmçd'È?·ÛCÝûH`?önõ›øïk@7Áe¤8?ÑÏ3"f×z¿ßSȟ@¢‡¿ÞµÿÆÜ¿Ñ	žD#E¿áÎW±—½!¿Øµ€ëLê"AGNbll3FGL J0208.6+3522MS 0205.7+3509?ïýíèÀ9?ìƒz4*Õ?0¹"À‡?ìƒz4*Õ?ïóiƺ†q?Y@ÇÉe+?Y,rÌëž|?Y@ÇÉe+?ïõ"˜9?UéïòêŒ\?UõÿæʍÏ?UéïòêŒ\?ï硍ÀË?F}	ڄ)?h^r>\å?F}	ڄ)?ïü4
Ο¶?3%ž`qS÷?>_'Klq
?3%ž`qS÷?ïÒÎ=²Šy?u¬rg» ?v˜á<¸C†?u¬rg» ?ï÷§Ùù0-?bc<—‹?P°LAÙµ…?bc<—‹?ï ×Ùu'?pBiÌbç?‡Ê9;äFa?pBiÌbçAGN4FGL J0209.3+4449?ß;7™…‰À/À¯¸kÀ:r™A…ŽÀ<|á®ai@ fŽ›ê'?ü€0ŒÅÛ?Äò™åﳂ?»!²,b‰?önøÜP@@[Èµ¿ÈE»K¿ç³l|*¿Òf'åK†¿ß§üaåοà••_x6¿Ñ,Ó}kÃAGNbll3FGL J0209.5+44491RXS J020917.6+444951?ïÿ=þj?
Ra—àjV?@8¾Xz_?
Ra—àjV?ïõ¡ÊÀƒ?TϱӘ™?T¼j›Ë?TϱӘ™?ïúãª+Œ?3·/ˆ?DqVÕA|'?3·/ˆ?ïø]ì@/?3à´Xê3?NˆPÔ0.©?3à´Xê3?ïÿ4·}ìP?¤5/Vê?iš—'?¤5/Vê?ï̞kæX?"÷ÇÖÏ?y°É쇥?"÷ÇÖÏ?ïý/6	¸?=¢ÂÈÂ=S?7þ…ì½|Ô?=¢ÂÈÂ=S?ïèáDAè?S!@òÚl¹?g»Â7lY?S!@òÚl¹AGN4FGL J0209.3-5228¿Ó¾ˆƒi"üÀNb$‡wÀ8—ú…l»ëÀ;º•µßJ~@cŽy*
p?üêzAå}ž?¢î½¾h?žFøaûó?øù5
£Çñ@ Àžìå?Þ5ëŸJÞv¿ÐOõ
ÙwÖ¿âi%]‡›¿Ó­vÛ©‰|¿àKm̌¿ÖG EDØ¢AGNbll3FGL J0209.4-5229PMN J0209-5229?ïÿ>ø'2?7b¡?8 ´»M£?7b¡?ïöö3£pˆ?TÁ>·hg?R˜•c7?TÁ>·hg?ïíc:~\?q)ûÕ
¢]?bœÅìƒù?q)ûÕ
¢]?ïþ‡¨ç{‹?ždwGS?'…sewt`?ždwGS?ïýêBÔj?+8/ø«½??0­ðY+r<?+8/ø«½??ïێý<ø?s—d¬Æ%Í?r8C¾ô?s—d¬Æ%Í?ïìÿú"â?u˜ÎìU^ò?c̯-ó?u˜ÎìU^ò?ïþC¥¤ÈT?#'
}½m·?+Å¢\0|?#'
}½m·AGN4FGL J0209.9+7229¿ïü-\|@%àŠï³À:ZÄq´xÀ;ïËWÇ@[ZÈ£r`@›ß>¿Xp?ÀºAYç|ü?Ñr»´K¢@í¬«ÅH@;OŒZA¿åå¥ `r±¿Ý§4ø/Q&¿à½¥6Ü¿àŠ#opÑ#¿étNáºo¨¿ïÿ¤àõx¾AGNbllS5 0205+722?ïj©Cè¯?Ÿ«´+ô®?'ªÞôN?Ÿ«´+ô®?ïèeq@V?rCó‹Í?gšŽÐ'¡5?rCó‹Í?•Ž‹ã?™¤ý«	§?¥E6§AÌ?™¤ý«	§?ïû	ÊóÈ~?0‹«ê'=?CØԈGJÜ?0‹«ê'=?îõe""×I?—Ü…%y¾? ©¦Æ‹o?—Ü…%y¾?ï€I՝<"?¡kÀƒÃ?íŠŠò‡¨?¡kÀƒÃ?腼¾ñ(?²v@L€:?Íé
ˆ;_?²v@L€:?ïéõ"gš)?X‰N/$f*?f
ÝY-?X‰N/$f*AGN4FGL J0210.1+2518?ïþZ'-û¢ÀAWÿ›V2À:ã쮤"À<_ˆü"d@ 6Ä÷@hÑ?ýéXÎG ?Èív{†'?ÂèSX?úþ³†ªª@ †ó¤§ë¿ïŸr÷na?ïD1Rˆc¿½"ëYÕ´R¿Ú`χã¿Þ»S'Å@ç¿éþý×0ÓÝAGNbcuGB6 J0210+2517?ïþtp{yY? –¾¨	?(¸ú*uù? –¾¨	?ïí›'Òñ™?c}™c^ä-?bdØ&//<?c}™c^ä-?ïã`·Ã{?v}¤Oñ?lŸp)ÿôë?v}¤Oñ?ïÕ㖊<ý?W}P¡¤É,?u4ž´µÑ?W}P¡¤É,?ïö~§ÙUû?Le­¾"oˆ?S°`'Úm?Le­¾"oˆ?ﻒu8h?…œà¢¡èä?b¾Z~?…œà¢¡èä?ïÙ4QôÇñ?y­…pÅ?se×
Ûc?y­…pÅ?ïIš6ç6Ÿ?"1ó³7š·?–̹(@–?"1ó³7š·AGN4FGL J0210.5-1445?æ<CŠÛ7ÀPõ!…Æ~À;0|ý À<®6Ýß@Š
D·)@í¤Ûìû@?ÉøǼ톬?–C<j¿fˆ?Ê:ÜúA@S>"u¿ç`
¹(*¿åõ–àVÂZ¿äÅêà´
^¿ç²PIÄo0¿ÂªÍ‰
UC¿ïü¨AÓ	'AGNbcuPKS 0207-149?ïýíôD	?&9¥¢¦B?0^µ—¨?&9¥¢¦B?ïô5¯?`84 ­Ì?W"á€èbŸ?`84 ­Ì?ïëtÜ\?ff_ÜXš?d‹#cJ:Ö?ff_ÜXš?ïÿ4¨Ež?^Q?p@œP?^Q?ïüáwñ9?6ÏÑÒù?8÷åz?6ÏÑÒù?ïÔïBdöÇ?vàŸÁ<§ü?uˆ^Ê{?vàŸÁ<§ü?ïå×òèå?pšÂ8G7Ù?j(ÜÚÓu?pšÂ8G7Ù?ïúŒÝS)?@BTzëµ?E̊=™~e?@BTzëµAGN4FGL J0210.7-5101?îô8÷m_ÀNã
ⴖÀ7Žî&¹¨-À;"Ë7¡W@ª¢%.b¿@é¾?kOÚ?"yy»n?µÒÿTÿ6@!þÃüC²Ý@7hÿóÀ­¿Ï'X&`¿áûúëÄ	¿ä¶U⊤3¿å桇N¾¿êÕ#³co;¿ïÿÈ¢› ÛAGNFSRQ3FGL J0210.7-5101PKS 0208-512?ïíÀ½mÍ?]ÔNpƒO?b?BáS#?]ÔNpƒO?ïîJ¹ÏÂ?pŸ
é³Mx?aµF´÷nc?pŸ
é³Mx?ï—mH>{?¥ˆ1´¥?Š$­÷YJ?¥ˆ1´¥?ïüåÊ'^œ?/q›ß²õî?8ѯøèû?/q›ß²õî?ïå¹7™ŸN?bƒ¤P1?jFÈX¢B0?bƒ¤P1?ïË`ï-‡?ÎxQ(W?zOˆ"f¼f?ÎxQ(W?)2ål?Œoå-E?ˆu¨÷Ñ?Œoå-E?ïïúÖS?YÑ(§)Ó?`çñSWR?YÑ(§)ÓAGN4FGL J0211.1-0646?ïŽrünG~ÀO.œË}AÀ:­ß1S_À<œÂ?«º@bWšÆ•P@ˁ½?ÁÛק·?úàe8?ÝÃn_E°@Õÿ¾^Ë¿â<Þ1;¿ç窟ѿÐ?Þ½:3¿áólß&k¥¿â;‡•‹¿ßPå€wߋAGNbll3FGL J0211.2-0649NVSS J021109-064551?ïþÊ"£n?݅ځ?ö?#]ÔYã­?݅ځ?ö?ïô㬄¥?[(	Õ[ª?Wú8O¶
?[(	Õ[ª?ïùL5ýVÇ?T¢K%^?JÏ(1 5?T¢K%^?ïýÙíû#U?V׃G«¨?10ÆS7h?V׃G«¨?ïþ!•¦ñ?$Z[>Ñ ±?.Ýâ²ù*?$Z[>Ñ ±?ïÔ°A·ì|?wñ]bu,à?u§ß¬j?wñ]bu,à?ïúO©'è?`¾±¥*Ñ£?FÁZ•sšÊ?`¾±¥*Ñ£?ïùŸ­ý I?<@¶"
?IGa<Œ?<@¶"
AGN4FGL J0211.2+1051¿Ë¬L®ïJÀG¯Š	ÞÀ7³´&ÚÀ;FÀh Ó@ìœf}t@hG,{Ä?—œM9Tñ…?ªÑÆþùè@¾×@Än@çuK[ž?Á]GXÚ¿Ý×Êâfçì¿âÿp"§Êµ¿àúLÍ8,—¿äÀD=Njſä.¢<ÖAGNBLL3FGL J0211.2+1051MG1 J021114+1051?ïü\§ ÃZ?:¸¢PtR?=Äao…?:¸¢PtR?ïóa}8Q?^Ã¢´?Y=YD?^Ã¢´?ïåÿ™'Ú?pëWXTËv?jû=œÖ€?pëWXTËv?ïüÒ ý.G?(T狂x?9nö֘\?(T狂x?ïý¼¶ÕÃ?)FoÎ3?2HüzW?)FoÎ3?ïÎÄ>€;?€–>óì-‰?x󝿶Ì?€–>óì-‰?ïãàãbÃø?zÿ±!ßÇ{?l¼Øoº?zÿ±!ßÇ{?ï÷	\}·ï?F¼õÇsmÊ?QíGIHQ?F¼õÇsmÊAGN4FGL J0212.2-2559?î‡cÑቝÀQú¢‡~äâÀ:þŒjÜí¬À<·†«€L@´Û%«
Z?ý#·ÊÝ"?ÉÈ#š¹Õ#?½.ëÐÉÃ?òðñõ{AÀ@¤ýÒ(V`¿Á‡
`V,¿êHº–i?­¦ŠÃ½Úl¿ã¤ÁëÈ:—¿ÞáAäP÷ê¿ÖޏØO·ÎAGNbcuPMN J0212-2558?ïþ¹öJ8w?Ýn&k?$`›§À?Ýn&k?ïôÂ"Z©?Ypa2?VÄ{TÀÔ?Ypa2?ïòò§4Ò?U?ÐðóÔ?ZÍ-HLE?U?ÐðóÔ?ïú¯÷)Ð?.]ýÞ5¥?E@"یë¶?.]ýÞ5¥?ïýôk»ÿ?-]FÏäÑÁ?0\ qXM?-]FÏäÑÁ?ïԆÑ&4?+=ª')?u¼—q†¿?+=ª')?ï÷jôõ'?\"1eÖ±?Q+ȆÈ*Ù?\"1eÖ±?ïï,ŠÄáé?QÇÀ2	@?`ÓuH܆·?QÇÀ2	@AGN4FGL J0212.2-0219?âGÛ`ZÖÀMDÁ~ºñÀ:åG5H·)À<£zm"h@:iàCw#@ƒýP"WC?Á·ýO0À¿š6°¸'xÛ?ÕÚSÑä@…ѳ'gq?ïçu$oK¿â#Ê|"¿ãÍug‹*¿åPâÁ*Ø¿Ü•ƒŸÝ*"¿×¶ %#ûÞAGNbcuRX J0212.3-0222?ïÿµÚþû?S>vÉý?I?øAÄÿ?S>vÉý?ïõè K‹?WžûæLO?UÚ/}pj?WžûæLO?ïøãÀüh?:v›ÐgA"?Lpü5½"?:v›ÐgA"?ïý÷՝R?ì\»°?0AS§E?ì\»°?ïþ…uº9?#ý`"^òo?'¨¦|¢$g?#ý`"^òo?ïÑÙ]2?|âµ›Ç?wpqƒƒ3M?|âµ›Ç?ïøÐ	Üçf?U–ѽ> ?L¿×òsé?U–ѽ> ?ïøŽfWd?>ƒŒKú?MÆeª[Å?>ƒŒKúAGN4FGL J0212.4-3502¿ê4xm­‹ÀQ¾¹¡vÝ­À:Wõ ¨ìôÀ<«©f–7@j¶JU @3T¦J'?¹ÒœÅsE?ƒA©ÝMg?ÉÖ§.ë{@ƒC¹=N?ÑEœš*
¿æ·½ ‡_¿Ù`ÈWG¿ÞAàËy¿å³2'#ƒ"¿Ê	 :2*õAGNbll3FGL J0212.8-3504RBS 0292?ïüÿJ6?+$U46?8­G.¡?+$U46?ïöÌ×xf2?T«•"1©?RfQ²ûÿ?T«•"1©?ïøÝÓ@•ƒ?QLòõB!?Lˆ²
øj?QLòõB!?ïüҀà#?&P5‹¨¡?9lų?&P5‹¨¡?ïü#G?1´œОg?>ç,úI&ò?1´œОg?ïÚ(%@´Ú?sûÝj®'z?rëí_¥"3?sûÝj®'z?ïö1Iõd?iHOjB‰R?SÍ=Zˆs?iHOjB‰R?ïùN¥??0v'òë?KâÇԇÁ9??0v'òëAGN4FGL J0212.8-2721?—ež·³—ÀQû†ìë¯À:Ìb¯!ÁÀ<·îŠŒ¶\@2œ"uÃQ@CTc.£?Áö
HX^f?¨Dͺ]‰s?ä鋧i@#f•á(N?ïµÖ±R¿×s×}ªÐ¤¿ãZŸ2ਿé·?Ò}涿Ì=$ä
d¿ïÿÿÊPËAGNbcu3FGL J0213.1-2720PMN J0212-2719?ïý²Ve"«?&Òx-­Ûª?2mKŽ)¥²?&Òx-­Ûª?ïõ;‡?¥?Wéæ»ÆÍ'?Uáˆô@fE?Wéæ»ÆÍ'?ïåÚùœtÑ?gV)9'«2?j%+1–Ú?gV)9'«2?ïüÈùéÕ?&¦µŒ´?9¿÷h"ä:?&¦µŒ´?ïûÓt%Û?<Á+¨S1ˆ?@³ÅÖåÕØ?<Á+¨S1ˆ?ïÑ(	ŌÎ?þ.øȟˆ?wkû&؁?þ.øȟˆ?ïÊ}«ì`?}›ÃÑ?zÁ)øÄCß?}›ÃÑ?ïóÚ­‹?M§³x–š?YÖJRs:@?M§³x–šAGN4FGL J0212.9+2244¿Öˆžl´&ÀB/ü~k?êÀ9ÐK¨ñÀ<<µ…ˆj@ð2¸9?ÿäçUO?µó8ò9î¹?¾·]¤ËÑÐ@
/»¯n@õÆžh5¿îÑҀ@M?ïæ#J‡ã¿àËÂFa
¿à¥0 Y;Û¿ä<zo1ç¿ä÷ƒŸ‡DWAGNbll3FGL J0213.0+2245MG3 J021252+2246?ïþˆÏ¥wÒ?"AÃ+3?'sè§Æ2?"AÃ+3?ïôóµûú?UÖr'?ša?V–
*è?UÖr'?ša?ïðI?hw¦©y@?_×ûª\ì´?hw¦©y@?ïîÀ¦_?F†¿55h?a?Yw¹¡¬?F†¿55h?ïû–S5~‰?>äùšÍ?A¦³³v9˜?>äùšÍ?ïÑ'÷" '?z3‡˜òt?wl #Hž?z3‡˜òt?ïâó®t-`?w•¿ëÍùà?mQ'3¸s?w•¿ëÍùà?_‰kW?pµ|@Ò?€Ð¸m\^?pµ|@ÒAGN4FGL J0213.8-6949¿ç"±/Y×.ÀFÔ×ðí=†À;!ö'õ;À<Àµ™ª`'@"5Wâ¿þ2?øáv<?A?ɂý5uWÆ?¶.Ý8)è?î'gbÂ*@ÞÇÌÿ¿ï³ «Ü'=?ïõf4€¿áÁçâÒɿ؀Q~Í»_?€>—•]tпârá锄AGNbcu2MASS J02135882-6951360?ïÿWûOÓ>úÜÁ	?©ÿ|'Ó>úÜÁ	?ï÷u}Ž(Ö?RSÍ^¤op?QƒyE?RSÍ^¤op?ïö°ïݯ.?DÁˆ»Q?Rž ¤Ö²«?DÁˆ»Q?ïÿ+m'[ö?aINnAñ?'TˆÙl¥?aINnAñ?ïÿš±`y?x:"UŠN?	S¤ˆ6!?x:"UŠN?ïÜU½ˆ"?6ç\q?qÕ!7Ê®?6ç\q?ïõ›ª‡?`½ÇÑ£"?TÉÜda¶?`½ÇÑ£"?ïýpI¥K»?.É·uø‡?4}±4ë&¶?.É·uø‡AGN4FGL J0214.1-4733?ïÇrøÅùõÀOù
¿cíÀ;€£n.²À<ê»ð¶ù@ qâ;žè?ü#æt=¿~?ÝΟ C×Æ?·_Kêå?Þ±]û³À@ßyw»#¿ä¾¡@W%¿ËâäfF…ö¿ã[ºÜ	€²¿ÍÍâK ¿ÛV,\\׿ïó±"L["AGNbcu2MASS J02140989-4732357?ïþê>«??¶Z?Kïú?!\‡=é?¶Z?Kïú?ïöëÍ(?UóiJš¤?R)î&Àß[?UóiJš¤?ïéx89Ç?p)‰ŽØ?f‡Ç·¨2?p)‰ŽØ?ïþV
9	È?x§ð>?*Ÿ*ÀaN?x§ð>?ïÿJ–"ÄÔ?ü??šën?­,{Ið°?ü??šën?ïÚ=j¼ò?rÓ9¡U†?ráJÀë?rÓ9¡U†?ïïÑÿ3Ü?lЛp)Ð?`.ˆ)ô_?lЛp)Ð?ïún´"?=õN
]ŽO?GöDÓï?=õN
]ŽOAGN4FGL J0214.2-7025¿ÜÝ&bP"RÀF[ÕìlÀ:)?—Å"À<vׇ:òD@Å´Júz@Ñí@	ÛK?¹g'Ñ_Ú?°¤žìzù?ðB'!¬øò@?q¯ðž¿Ü€'q^çí¿ç@D"­Ç¿è'&ëý¼¿èéé¾4ú¿íA8D,¿œµÐ±Þ´×AGNbcuPMN J0214-7027?ïø¸<ê8?HPáá#?M	
O?HPáá#?ïíØò0DÒ?lþ²tõ1?b'
Ê;͉?lþ²tõ1?ïN•—ßä?†üòYyC
?Œ¬Z ç?
?†üòYyC
?ïëOÚ2æÝ?RXtbä?d°%ÏØÒã?RXtbä?ïñ+ °…?]n&*4}?]©ÀFV
?]n&*4}?メ;E?>?…ÛHüÎ;E?€[q&q "?…ÛHüÎ;E?ïÊ¤9ÁÔ?‹¦…¾¯ùc?‹ÍVûÞ^û?‹¦…¾¯ùc?ï2	
Œ[?çõêž?™¾Ü·n¹?çõêžAGN4FGL J0214.3+5145¿é0ó;ˆÀ"s2&ÄÀ9÷kÅJøLÀ<C:8
2‰@ ›ú©ÿÃD@ñ›¹.Š?®CµâO•ê¿´'HnXÎ"@7E«I@ÑZÚôã?ïã)›üå¿æ™Sù|X¿ã«xßdÔì¿Ô±qÝ=r¿âkí>\\!¿ÏÑß[DÊAGNbll3FGL J0214.4+5143TXS 0210+515?ïýu‡c?(&‹	cˆ¥?7ÌTüUì?(&‹	cˆ¥?ïèš@*	?e&ߧӕ?gúeêqº?e&ߧӕ?ïô"º6È?aCí¦;?V֋'<
A?aCí¦;?LG'r?]YÏËcz?€ÔîM]Ó[?]YÏËcz?ïú¤ÓÎ8?@Û¯J×?GámPÁ½p?@Û¯J×?W=î<?•6Ù­qB?Qª>Bàï?•6Ù­qB?ïà‰Ö`§é?y—
ß\:v?ov)ÖQ֘?y—
ß\:v?î[eõÓy?'-'y?ªI¦ïÆáv?'-'yAGN4FGL J0214.4-5822?à眄¹hÀKÇߏG0@À;}ÂO›HÆÀ<òÿ4(%¹@\E*¯}?þû˜\'·Ö?ÓG÷›,–·?Ԙ\bq?ýëWfï"b@
ôù
†¿ïQ¶
éh?ïÞ'bEo¿Ü—û3èe¿âÎcûR¿æU.enâ¿ïÿü¥¬¨AGNbcu3FGL J0214.7-5823PMN J0214-5822?ïýÖê\¤?0š¾\þj?1H«Àïmñ?0š¾\þj?ïö§TÿG?U™¤Èt?R±UݶÐ?U™¤Èt?ïµfý÷"r?{±²F¼
ˆ?'¦@"G'}?{±²F¼
ˆ?ïüfFA>?&s]NPT
?<ÍÎáZ¬ò?&s]NPT
?ïþˆQÜI?%çIJ
#?'šÞEh?%çIJ
#?ïÝ;ùð
X?rÕj¥š>¿?qbëÎö?rÕj¥š>¿?ï¦f*E<º?†ÞzS–­?†fuxÿ¥z?†ÞzS–­?ïô;Îã''?M#*·ˆ	?Wˆb"f«8?M#*·ˆ	AGN4FGL J0214.6-4333?×xÕñ°ÿ3ÀP Ž4À;ïiÃèø|À<ü]¿Î·‰@"Ù¾9a«?÷ Â'Æï=?ÚrÁ`'?²Ì)cы£?×"ªú¿ú+?üøÃñ11?ï¨HSUèj?ØãŸAyG¿êcnÏÁsÓ¿ÉÕ	‡=K¿Ðu¬¿ç<¿Ç""7ª¼,AGNbcu1RXS J021439.0-433319?ïþŸÎù%?.òãÁ7b?&7š3?.òãÁ7b?ïôÁ€ñà‹?Z¤·àüŒ‡?V|ý®KjR?Z¤·àüŒ‡?ïç"õ^£?m;¬ð‹³E?h÷Ý2|Õ@?m;¬ð‹³E?ïüR³E?/'nF–|®??¥hm*û?/'nF–|®?ïþ7Jïè[?,'žu:·?,‹PœR Ü?,'žu:·?ïÓºÕS"?z…Ä›í>?v"•XM¾4?z…Ä›í>?ïÛiøí;?|)fêÈJ?rKŒ7‰?|)fêÈJ?ïïÊwÕF?X<·êˆ6ª?`5ˆ}`¯?X<·êˆ6ªAGN4FGL J0214.8-6150¿áj`û‡94ÀJN(ܘëÀ;6¬7+xÀ<ÄR)˜¾@Pþ39é@ˆwîN&Õ?Ð|³úîÉ!?Ð>͛(åÒ?öýã¼Ó[?î—õøó¤Û?ìŸÝJÉQî¿Ìôœ_ÄW¿å`¿'țæ¿ç[`m~¿ïÿ Êƒ+?ïôìp×±AGNbcuPKS 0212-620?ïÔ¤+»<#?|Ñ –ï?u­ê=ÞÎP?|Ñ –ï?îÜ>¤wæc?°‰»'–.Ñ?¢<¹]€Ð?°‰»'–.Ñ?î¥Øʺy?—Ê0°äô=?¥¢sQÄ3o?—Ê0°äô=?îæõR'A?Š43R+µª?¡ªÙC8ö?Š43R+µª?ïÂ!¾tM
?'œÕÂÎsü?~ï Õ§­ª?'œÕÂÎsü?åìA.§?Ñ~e©°›œ?Ô'Òá}¢²?Ñ~e©°›œ?íDéÝúƒ?¡G¸97œ3?µØ·ˆ¢8j?¡G¸97œ3?埼ô;?»¬ÓnbÅX?ÔÀ‡Âà‹?»¬ÓnbÅXAGN4FGL J0214.9-3722¿ï@lüq¥ÀQip£×
=À:Ç	á*QãÀ<¡ jْ®@»ˆçÕ@S3¹jð9?ÇàáÂ'W]?±>lwL"?äq|^ö/@¹U¹ÅÞò¿°ˆUà˜lÚ¿èæÙóü¼¿èyÞp¹&¿ïÿ·äkO?ïîÑk%¿ïáûÓJ•PAGNbcuPMN J0214-3729?ïýªG¼­?b_Ø]ô¯Ä?2­Â>ßÜ¢?b_Ø]ô¯Ä?ïö'Ö±Òö?S»H/4œ"?RÚRÿNÒ½?S»H/4œ"?ïË*PØØ?}"Øz"?zuê¼Æ 0?}"Øz"?ïÿêÏþ@É>ápamS>å/à=CxN>ápamS?ïþ÷mp'?'؄¡=1Ç? ‰';«ÕÕ?'؄¡=1Ç?ïÐÙd"[?'CªzÏ¿?w"M´B¯(?'CªzÏ¿?zIÇ.?ƒÕ݆›Þ?€™mÏdJc?ƒÕ݆›Þ?ïþ|_wö?,Æ6ÖžZ?(:¸®6?,Æ6ÖžZAGN4FGL J0215.3+7555¿çå=ð..o@+ÈÂ?«ºÀ;)A® 9À<˜?gôÛà@"cÑeõ?û!DˆÆ¿?ËlØÆU9m?ÀDc²,
?õ#|ÜÊpÒ@'ÇœŒ=;¿ïÿîͨ"ß¿ïüúAzÓ?ïÿÿ^ðP`?y7»ûe³Û¿å&Õ!/$±¿k7¯çUAGNbcuWN B0210.3+7540?ïþë­Z
4?IÉ0$?Q?!E+óˉt?IÉ0$?Q?ïï"$ö?aZÉÆ!RÜ?`ÝÚÝwè	?aZÉÆ!RÜ?ïñûµ:y?_•ßÙü?\•ØöM
?_•ßÙü?ïàs±N§?^Mh¾(?oŒNçs‰?^Mh¾(?ïþc+>?"÷?ÂíEe?)È x1?"÷?ÂíEe?ﳕA¬Xõ?‰ÕH5<¼Ž?ƒ¯‹úÆÄ?‰ÕH5<¼Ž?ïòÖ8}ÂE?f·ŒÇï°a?ZSC´E§?f·ŒÇï°a?ï©)¦äÓ ?|Z¸!ŠåZ?…µ–T‰§Ü?|Z¸!ŠåZAGN4FGL J0215.9+0300¿ïäeh±ÀJÏO'õfÀ:Ÿµ<OÀ<wRœ…e@›	³Ýè~?üðÏÆ|P³?ÍJ‹¼[?ÄØOø:ä­?ø¨Øœ
è @)_SL®.?ïþdŸfã¿èK7 }£ð¿Þߤ¬ó¿Ò¤^Ƃ;¿ævîÿ|¢h¿ç,Sæ1!áAGNbcu3FGL J0216.0+0300PMN J0215+0300?ïþ"'9'Ø?óv¾¯Ñ½?&ÇÚª®—ý?óv¾¯Ñ½?ïô†0ŸôÁ?X'.Cêx?VóžmŸÝÚ?X'.Cêx?ïð«§õ87?]|´_Y^?^¨¯æÔâ"?]|´_Y^?ïóou¦Í?=¾Žà?Y!|ئq?=¾Žà?ïþî^(:˜?ÅZÛÍ?!!Á@¡ÿ?ÅZÛÍ?ïϒÜ)ûÁ?ˆÖˆÏP?x6'ŽÃu?ˆÖˆÏP?ïßN¥]$Ò?uKi€7K?pX­5@Ë@?uKi€7K?ïà˜ì |¸?ZGÇFÕl?ogt ð-?ZGÇFÕlAGN4FGL J0216.5+2313¿ìXügçgÀAÍ®_ú;›À:'{&ÁÀ<deÀN9I@ º¦'Ço?û)—Ãք?ōK±?Ç@÷Ií@Z	`ÑÑï@=*WíR¿·²Ãa>3¿ê‡/3Ê1è¿Øì]Ù¤÷¿ÒHj|öu¾¿à¹Ã_eÁ¿âsè/(âwAGNbllRBS 0298?ïø¤íñƽ?Cܾ
XÿÌ?MlH3òfê?Cܾ
XÿÌ?ïïönË~ˆ?b­â|èƒ?`	'\\ïê?b­â|èƒ?ïêã'
Ç?_f	Œê
?e
l˜—?_f	Œê
?ïàt¦´Ï?PŠ¦ððǗ?oñ‹+ðYQ?PŠ¦ððǗ?ïé6AI?_´ÁdÐr?fàèôYÞ`?_´ÁdÐr?ïË¢(x?zŒWòDRƒ?zuw§\Ÿñ?zŒWòDRƒ?ﵚU'?†Ð
>Äñ=?'™jÂeŸ?†Ð
>Äñ=?ïe߯lXˆ?/; LY«?"D
ä‹?/; LY«AGN4FGL J0216.6-1015?à1ˆŽ.sÀO䦰)(À9¯'OH<°À<Sû!sî@´¹¯ä‰­@ÑÿÁìžú?²"¡9öñ¹?¶"^—&@rá& %9@/«$ÜX[?ïØ~>õ3¿á[CÝOÒ¿â(ey×\s¿à峃O«9¿æN'b™R¿êdüAGNbcu3FGL J0216.6-1019PMN J0216-1017?ïþöЬU^?¡öôl¯? 'ó‡B¼?¡öôl¯?ïô}1À(?^
$Èi—E?Wá#0_Ý?^
$Èi—E?ïôFâñ?a1‹i³S{?Vár£˜?a1‹i³S{?ïþá
1Ó?Z=)??&!ðxðBE?Z=)??ïþòqՍï?úM	€? Øá³	œ/?úM	€?ïÖÉo?|3̀4º?t›HZ½§?|3̀4º?ïÞ§ë–çc?xäÁÖ"±?p¬
K馍?xäÁÖ"±?ïý")\®?%
"*D?3^µ'¯M…?%
"*DAGN4FGL J0216.8-6635?УCf‡ÀH2â\
WÀ9ßæÆsxÀ<A,…šT@ˆ€UÐÁú?üšÊ¡yaì?µ³›ÎR2þ?ˆÇ#ël @1'o°'@Oìú"±'?ìÕsd{ª›?Ä;å'Ûg¿Ýá\†Ô¿Üi.âìsÜ¿âžaÔU¿çž|øy#AGNbll3FGL J0217.0-6635RBS 0300?ïüNÈ:û?;«ü¢oW"?=‰¾…—ÿ?;«ü¢oW"?ïó†-ÕD?W«Z
Ëñ4?Xó¥…áX?W«Z
Ëñ4?ïÄ3]qí{? 8̧œ?}æQR©? 8̧œ?ïë,LþÐ?K²_)Ð\?dóÓ°Aë?K²_)Ð\?ïóã./Šª?U!8J¦l¾?X9¤	^Ì]?U!8J¦l¾?ïȱ'R?ƒÝPi?{§|qò¶î?ƒÝPi?ïNö¦B§ù?"þ,áÍtn?–!+<ÒjÝ?"þ,áÍtn?ï²»ÉÈG?o(AŠtV?ƒQ—_?o(AŠtVAGN4FGL J0216.8+0510¿²×¼o"}úÀIÕg–ØõÀ:¶ÿݛQ*À<"YÙU@ñiî†0@­õcÄËw?ÂN´XŒ´?W.0ͤÏ]?•ü‹^öä@…>œÈÎ?ïóg ù	l¿æ¦I«D¼È¿èZ9œÙ¿ú¿¸
¤ô–•X¿Ýв_Ž0¿ïþÖ4T›cAGNbcu3FGL J0216.4+0507NVSS J021655+051018?ïü\·»îƒ?0¡"Ð…v?=@i×b£?0¡"Ð…v?ïõ¶É]à?WZq'z¡b?T'lÛËÅG?WZq'z¡b?ïñéz5-è?L›ŒqEwî?\-wg ?L›ŒqEwî?ïûZ+"ü?)Ô(ä+'˜?B—߯!q?)Ô(ä+'˜?ïüz5¿ï3?2½DŒ[?<.Q‡"+ï?2½DŒ[?ïÕê£uˆ?yFVLœ?u
ž'È\4?yFVLœ?ïðv5Í}ˆ?gÏïN$xÍ?_"
O@…?gÏïN$xÍ?ïñUØ+ø?Lf‡÷¦?]TP,œÏÝ?Lf‡÷¦AGN4FGL J0217.0-0821¿Ñ‹v,úVjÀO2q`•l
À: ZUÖÀ<t¿û-2h@¨0lYoˆ@+œ›¬™Q?¼ð¢…?À•ÙE¬¯@Lz-È?þ66ò?ïÜ3<mn˜¿ãb€u¿å0éý_;пåv•ˆ'á¿çŽc_öµ©¿ïð"¡!1AGNfsrq3FGL J0217.1-0833PKS 0214-085?ïø~«Îò¹?KRõ»ñlÆ?NPxäÛ?KRõ»ñlÆ?ï®`(ðË@?',Ú¾!ð2?"gõÔ£Eî?',Ú¾!ð2?︾"à-c?€:-û'?Ð[
;?€:-û'?ï"k…	>Ã?€P¥}?›²Wøï¨?€P¥}?ïªJ³FWÂ?…J¢^»×o?…mS<(o?…J¢^»×o?îFÄýlõ?¶&4pj¹?«"°+Äcy?¶&4pj¹?íÃUL/$þ?¨bÁù©À?±åU<ý'?¨bÁù©À?êÊêY¥Ä?¨ ¿ÉF??ÄÔV™iÈñ?¨ ¿ÉF?AGN4FGL J0217.2+0837?â>^ˆfÊÀHQëcÉÀ8­43ä3À;é=~æì@¾»Ú(Ö@ì·M߆ä?¤	±ãÃ?¥]™@áÐ?ÿ¶¢Ù´;Ü@ÈBS6³Æ¿Ò¼ççÛF¿ãeøí½]¿ã»'Ê°h¿âë¹VÎBï¿å҉øÌ¿éJñáeAGNbll3FGL J0217.2+0837ZS 0214+083?ïþ½8–Z±?AÃõæ?$,x¡M—?AÃõæ?ïõj'TŒÛ?Vv®!®Ù?U*ÝI'Ùf?Vv®!®Ù?ïðÉ=æ?lº7è²X?^m…¾CR?lº7è²X?ïúÊr:Á-?7}އ`©?DÖ7a1V?7}އ`©?ïþV¸|z?$Ë=màË?*"v؇ƒ?$Ë=màË?ïÑïÒÇ?'¢£.?wqvøøT[?'¢£.?ïÞõý%bÄ?€Î>}Cl?p…z]"?€Î>}Cl?ïôPËìÊ?OlÊuÎ<?WÑ^œ`zì?OlÊuÎ<AGN4FGL J0217.4+7352¿ïÙ֚àì@(âCV–æÀ9͌æ,ðÀ;¨Ó5œ™ÿ@—Èe^ÿ@tŸM¡?²ÒRȤÉù?ºÒ	!¼¾7@Ý¥b$¸@
»ž8¥8¿uv×çvà÷¿æïÖòÀ|\¿ëhª¾¯þ‹¿ëÕjËOõ¿ïûâ~å¹-¿íÏîõì€ÇAGNfsrq3FGL J0217.5+7349S5 0212+73?ïÆÊ%—X?®¥²ÕËf*?|šíG'È?®¥²ÕËf*?ïëò͛Š?dþBuÁÞ?d
2…õ¶?dþBuÁÞ?ï•Îd"?‡¯¥²r&»?Š¿{֓Š?‡¯¥²r&»?ïË[)½+?g_D'ì§?zRkrÂÒ¼?g_D'ì§?ïÚõ›#?{E²§]­ª?r…w`¥*s?{E²§]­ª?ï"ÿ^Dƒé?"É"¹·rþ?‹(rN¡Û?"É"¹·rþ?ï¨@•5K?•íE_§ý­?œJ÷íYV«?•íE_§ý­?îŠåŠÖ*?—%%oÓ?§X¨."c?—%%oÓAGN4FGL J0217.8+0144?×=k†òßÀK5 @|ÇÒÀ8DôètÉÀ;¬šˆ¬âL@ÍVnjñë@FÙ='©?X,€«Oé?°X(àôÌñ@Èí_‹Î@ƒxOÇéc¿½ñ¾xÌ¿áU74I³¨¿ã¤ô xÆe¿âŽWF7ò¶¿æ~c³-¿V¿ìì¿0|uAGNfsrq3FGL J0217.8+0143PKS 0215+015?ïüÓCç"?2`yØj?9gVÔÚÑØ?2`yØj?ïó»p{_"?_|$¶¿*?X‰¶Ê8?_|$¶¿*?ïåŽ^Ê](?qPAÝ­11?jq¡h}s?qPAÝ­11?ïÿ4{\¤?
'h‹.?p™)íÑ?
'h‹.?ïþÒÏ"ðù? 3,ŠI¥?"Ó9óŒ? 3,ŠI¥?ïÑ,ȵæ×?{Xâäº?wi›¢üÐf?{Xâäº?ïè-å°7Z?wþƒb"â?gÒˆ">?wþƒb"â?ïþM#…|g?">:Zô?+-Ç·ž/£?">:ZôAGN4FGL J0218.9-2305?ÝàÏ"ÌûÀQt_®¼@ŽÀ:"WÀ±5˜À<žù˜òc@"ÆóÄÞA@˜Ã`<€º?Àb–P9?¦À#Ç‹Ö?å'"^#̹@š?Ĝý¿ÕfÓP0š¿è,ÀÞ'¿è2µ>»§‹¿àÀ;Ÿ=r|¿ïÿþªJl?äcãÏßAGNbcuPMN J0218-2307?ïþ-Ӏx¿?&ÃaÏÀm?-"Ƕ{'I?&ÃaÏÀm?ïö	Ï*N?V|Ú?Sìa}ùt?V|Ú?ïèBSâ€=?gVR™î9Â?g½¬£
Ö?gVR™î9Â?ïÿ¢Á¥@0>ùcÎZ³yf?O£©>ùcÎZ³yf?ïÿTk^•.?™"­Ç?r–†ÀÞ?™"­Ç?ïÙÒ}Շ ?viê[<?sÀ÷¯Œ?viê[<?ïù8?h5fϤæÒ?aJþH!?h5fϤæÒ?ïþÄLù? <D4–Ý°?'ãºįs? <D4–Ý°AGN4FGL J0218.9+3643¿ì7ƒžtc™À6ê1…ýÀ9œze ì	À;˜	ÿ÷@¥³/³ø@ʅ4-?¹¶ˆèœa?ǤC@Çpl@
f|¼A%@``?°Å¿Àß]ނÐ¿änôËG<¿å=ù*"é9¿çÑ`°D
¿í>"z~K¿ðAGNbcu3FGL J0218.9+3642MG3 J021846+3641?ïæ"
Æè?bN ´Roö?iÝòkò1U?bN ´Roö?ïôwWՈ?XyÆRzÅE?Wèòߑd?XyÆRzÅE?ï¦fˆÂ~7?~DªZ6ã?†f]Ù¯FE?~DªZ6ã?ïú×ÿP?3ýØMAì?G¸£(¶¶Y?3ýØMAì?ïÓÓe(‰ó?qš¨.#?vM¨ÂX?qš¨.#?ïÐg­IŠõ?mð|&?wÌ)L=Ä?mð|&?íˆÕƒ'?£†úˆ?³¹S僝œ?£†úˆ?ïßåO>pm?^Ö}—†Í?p
XKz5©?^Ö}—†ÍAGN4FGL J0219.0+2443¿êœ°ÞÀÑRÀ@ÿÊ}g3ìÀ:T6KìhÀ<]°<sMÕ@ {ÂqÔ¯?þBÙÏÏ?¹jàHª"½?œ}¿ZÑæ?åT*Ã@LÌQ#ß¿ïW‡Üóö?ïÿ˜0ã͚¿äQ™_â隿àcRµ¯z¿ÜJ±ŸIÜÿÁÈpMLAGNbll3FGL J0219.0+244087GB 021610.9+243205?ïþ"µ:E1?‡[¾p©"?&ĬŒ
Îé?‡[¾p©"?ïõìýU?UuX]u`?T&^ð™?UuX]u`?ïõúâ"&?IŠ³BÂ?T
;À¼ób?IŠ³BÂ?ï÷d&´äh?9ñ¤tYûÒ?Q7²›¶Þ?9ñ¤tYûÒ?ïý~¸+´?,ËÔLÿø?4RÄÆUÌ?,ËÔLÿø?ïÔ@g+æÁ?v@'E:Ýý?ußÌO?«?v@'E:Ýý?ïðÕ֔Ti?jÚvk‡±'?^TRŠ_î"?jÚvk‡±'?ïá_îýú?at¡éÒr¥?n îÈ¿?at¡éÒr¥AGN4FGL J0219.1-1724¿ïft€Û\³ÀPã9–ú'èÀ:Œ/•ïÀîÀ<€šl'p‡@74:DI†@ÖßZn
 ?ÀZâ9E›ì¿m;8€Éç?±cDë@ëÔZŠ»¿åPVY¨é¿æ%»`"¾Ž¿ç)%]‡š"¿Øë/þË¿Ôx=({¿ïÿÜßi‡ƒAGNbll2FGL J0219.1-17251RXS J021905.8-172503?ïþ'1ёá?q`ŽbœÕ?'ÜâÈ¡œ?q`ŽbœÕ?ïõq˜ëì?W¡s/ˆý?UΦ™lÛ?W¡s/ˆý?ïù%†TöÛ?;Òî[[7?KiæÓ¹­Ÿ?;Òî[[7?ïÿ7¸J%?e£¹t?ú:»ð0?e£¹t?ïþ"ÖF¦¶?Âþ¡ž¼?'²ŸªÙ?Âþ¡ž¼?ï՘©7Nÿ?Ð'{>Ò?u3«O
ìx?Ð'{>Ò?ïù=pÎÊ(?aã:³îL)?K
;ô{Ýç?aã:³îL)?ïýKXª!b?-DÐ6z‰?5¥;æX?-DÐ6z‰AGN4FGL J0219.5+0724?è«Óœ¹xÀH³é ÀièÀ:ôBŒüÀ<cÀ›f"@ YC=A@mY9?È/Á#K^£?'ûôW«7§?ÎõŒI$M@¶ÜuŒI?ï©iñ5aâ¿åÒ%fÁÕù¿è¼Çf[~¬¿Û¸‰ÿr¼`¿ä ~æ¿Ûš©CÛ¡ýAGNbllGB6 J0219+0727?ïÿ'ÔkÔ?¡t¡ÎG€?rºm<?¡t¡ÎG€?ïõ6˙?Yҏl§Í?U'iƒ<˜?Yҏl§Í?ïû$òu?0—
90?C¯m
ìêù?0—
90?ïý …1?l°ò7Íê?6ÿV÷#«Ù?l°ò7Íê?ïÿMû,þÞ?O%§"g?@žs[³m?O%§"g?ïÖËæó¿€?xþOÙX`?tš".Ãÿ?xþOÙX`?ïü<	¬¸A?E6…''šÂ?>±
Q">?E6…''šÂ?ïó¼DR/?I…¾Uí'?X‡x/•²˜?I…¾Uí'AGN4FGL J0220.2+3246?æ¸i OÐÀ:z|¨"2À:‰m–cÀ<QjúIݚ@òÞÜĽ@^ڀêv?Îj'ÅêÛV?Ô:è‰A@s¹»x³@øE×î¿¿à¶l¾o;ø¿ãt°¨©Ø¿ëMª½Ù>ö¿éx՟eæ¿ïÿå(
eC¿ïÿþÐñAGNfsrqCRATES J022048+324116?ïön8í²K?I'¿B®¶~?S#Žf"êy?I'¿B®¶~?ïñš¸H?`\<Í(ýÑ?\ʐ?§W—?`\<Í(ýÑ?ïy`O\E?ú~`)Æ?¡§áÚÖ?ú~`)Æ?ïßW¤¹?Ul@
ån?p@T\
[e?Ul@
ån?ïùû†ÉˆJ?O1Ys")?HãÜnݧ?O1Ys")?ïÆ©Q¿Þ?"tŽÈ/Y4?|õ«>báT?"tŽÈ/Y4?ïO6xÚSÀ?Ž°Cd¢??–0ߎú?Ž°Cd¢??ï
*p–ëê?‰ØpóFÙå?žº±çû¾?‰ØpóFÙåAGN4FGL J0220.8-0841?ïà&˜°LÀNúˆ&ªŽ´À;SôÁœ¬À<´ÚìJ@–@!–L\yþ?÷Π/µÐ?Ôê&yçL«?Óú†c±Ö&?ÿ'~þà¹@W#	ðCÊ¿äúTû½¿ïÿ"Þï?ïá³äžzª?ÒÈÌøk·¿Þ~½_ÇeÛ¿ç:d_¦ßAGNbllRX J0220.8-0842?ïüIñªk"?0"»u^¯²?=°q2h×?0"»u^¯²?ïòø0¹í]?`lÜ(?Zž
óö?`lÜ(?ïÜñïË=?oB@A9?q‡>ÇÍr?oB@A9?ïõê:­Y?DQ›Øg?T+Õ ¢Îª?DQ›Øg?ïüSǗ«?7L'' ?=aœ®;?7L'' ?ïÐ
EÛ"ó?yñ!½Uf?wù]@zw?yñ!½Uf?ïð1Ç«Ù?iE«ïQBþ?_Ŝ²Mú?iE«ïQBþ?ïêµÅ8Á?a^¬ßú­'?eJ:Ýà¿?a^¬ßú­'AGN4FGL J0221.1+3556¿ÔôÙ/º5À7|K	éÎÀ70–›¸XÀ;)ûbó@Žn F±ë@Çâ'@¸?ŽÁsR]?¨¿3\"ë'@(}@@ Qg`Œ\Å¿Ì/
3Å)j¿àå!×¿ågûý<a¿âý§*{ԍ¿èKABG£¿ãE5þAGNFSRQ3FGL J0221.1+3556B2 0218+357?ïûG}(Zù?A…ê×L+?BâM'?A…ê×L+?ïôjŽG?czŨÊÒ?WÑ+î±Ì?czŨÊÒ?ïÂsg"Er?ƒÐç?êþ?~ÆLR°{Y?ƒÐç?êþ?ïÿËoÌÂ>òhÍSÑ®>ú@;É*Ê>òhÍSÑ®?ïùøÊ+²¶?E^­ËÓ?HÖX·Î"?E^­ËÓ?ïÁ")¬»y?'¿©­ö¹S?6kt7'?'¿©­ö¹S?ïÃëk¯?"‰æj¥Ø?~x
/[EÍ?"‰æj¥Ø?ïÿ¯()ÈY?pxˆÔEe?5ô1–zá?pxˆÔEeAGN4FGL J0221.2-1312¿¨%¦ù@­¡ÀP4 {5À:ý‰»Ö"À<›óÜ܉@ÿB%¿WC@òa|ÚQ?Æ SG$צ?°¬°L¹l?ä܅§tM°@l6k!=?ã¬X]ºn¿æš·¦ÊÛ¿çuK;gµ¿êUü¡PÈ¿Èò]dŠ¿ïø^졬AGNbcuTXS 0218-132?ïýçì…FH?%ÑXœ¼Û?0ÀÞøäÀ?%ÑXœ¼Û?ïò[È8û?c–ߦ&nv?[ÓH¦‡Ê¬?c–ߦ&nv?ïÞï{ÅÀ‹?l/Þ=X==?pˆB(Îf9?l/Þ=X==?ïüåÑ«ƒÒ?'?ÙlƒRs?8ÑqñÂ~ã?'?ÙlƒRs?ïýÛtÒ²6?*¿x$âC°?1$XH¡º?*¿x$âC°?ïÌOH‰þé?|&`çta‡?yØ[ÎîG>?|&`çta‡?ï»ò¬QÏx?'´zóʓ;?Tï«©þ?'´zóʓ;?ïåüÒÓD?ad¾¦-x¢?jðe†T1?ad¾¦-x¢AGN4FGL J0221.5+2513¿ï0^¶³t¦À@¨û¼¾bÀ;>1ø .À<Ò2º¥@œ9í±?ûåɾ$"]?Е™"Ë×.?Ú3~݀¤*@
Ô'ܾ²@	G¹¢£ƒ}¿ïÿÿ" 5•?ð?ňP†€7H¿Ù¦¿<@x¿ä"éõҀ¿ïÿô!O…úAGNfsrq3FGL J0221.2+25182MASS J02212698+2514338?ïý­#¨ë?7'|ºF}Š?7—Î^j?7'|ºF}Š?ïíeÝe²s?aêmLÙª?bš"·#?aêmLÙª?îT
­œÊ•?  &Ñö¹?ª¿U!çÓ±?  &Ñö¹?ïÙ}b‰ë"?Wœÿ<§i?sAN¥¼©õ?Wœÿ<§i?ïý4è2?7ü {Gö?7f^È嬒?7ü {Gö?ïÃKi_ê÷?'³'ï3"?~ZK>,Œ?'³'ï3"?îëd¯?›…܎¬n?¡I¾ýæ§?›…܎¬n?ï}Îc""º?~ôÃz­_
?F3'"òµ?~ôÃz­_
AGN4FGL J0221.8+3730¿ç<çFB&
À5÷Yš¦	À:àÐd1À<m?!Î@iohی@êS%A)?ÒÇþÜ¿^$?Ø*Œ»º«¸?úÔLJémí@Édm<ïJ¿îLAœ''?êÿý¥\Æ¿åº<;ðq¿ãU]Œþ¿ïøª*s?qInAGNbcuGB6 J0222+3731?ïöWŹ³?T`þAiÐ?SPt`ž×?T`þAiÐ?ïð_£v½?`ä®t(è?_@¸ât%Ú?`ä®t(è?ïX«"A‡y?†ê×î¡°U?"ê{>¬ç?†ê×î¡°U?ïڋ¦´+¹?ZŽu:÷ó ?rº,‹ÍÞ?ZŽu:÷ó ?ïã7êi…?sâÈúì®?lÈú9Rk7?sâÈúì®?ï¥j§?"€wùO¦u?†¸%NW̧?"€wùO¦u?î•õ5ö?š;caÿb?¦®Àªý¨?š;caÿb?îØ/Óh"?'"«þ^ç?¢~EÅ?'"«þ^çAGN4FGL J0222.0-1616¿ÉYçû¯ìËÀP—æî·`À:'õˆ­¹À<8Uêî @éÐ[L¬×@GڎVo?¶é9"÷ƒ¿sâX'Ö'?×Vj…YñŽ@
mc-ת?íëw²¿¿åY àŠÄÀ¿çWeÂ|'Ì¿â€3aV\-¿åû]8À:î¿É_A"ÛAGNfsrq3FGL J0222.1-1616PKS 0219-164?ïþ°þ¡Aj?yáí*¡?$ð??yáí*¡?ïõ?Œvµ?Z^nóm=x?Uۀ§ÙÅþ?Z^nóm=x?ïø©Œ"Z?<ïóº&Zƒ?MYÏ&à¾Ã?<ïóº&Zƒ?ïþÚEÜ-=?YþÀÂm?"[¡ÿ™—?YþÀÂm?ïþ™«"R?R`c¹‰?&nE¥Y²ˆ?R`c¹‰?ïÔëa.æj?€õåÒ±®?uŠOn+?€õåÒ±®?ïø¨Ùtó?R"çÎ=_¼?Mù\TZ‰Î?R"çÎ=_¼?ïüžÊí	ê?-y'§ì¥-?;	¦'mPŽ?-y'§ì¥-AGN4FGL J0222.6+4302¿Õ¨Ò?05À0Ãúñ€À6¢7Q¥åÀ:°"±"L[@Y³Ã¼Wà?þPKŽz??¸ì^ý*?¦d'‹‹@Og+ˆD@B{Ÿ]©¿ºÆ}A8m¿ØPÜfrÑ¿àtÐ!#~¿ÜÈh¤".M¿â4áô|>?¿ßuAË|jµAGNBLL3FGL J0222.6+43013C 66A?ïö²#‰?\*S¼CÖW?Sœ=Óí?\*S¼CÖW?ïó£>ð?dý±^Ý?Xü¹œ½Î?dý±^Ý?ï–Â$…y?Je€—§í?ŠO~é 1Ò?Je€—§í?ïÿ@ü/Í?L¾r@´›?àqÑÅÝ?L¾r@´›?ïü—ø|ƒ?:,  þÅÀ?;@;™ùr*?:,  þÅÀ?ïˉD!Š?"Â8œ°à?z;]Õò[?"Â8œ°à?ïØ3Η/å?']Æd¿Ñs?sæÊe"?']Æd¿Ñs?ïÿ2órS?4x›WTÄ?¡—sãà]?4x›WTÄAGN4FGL J0223.0-3447?×ÿÝá:ÀQ>þqŠ†×À:ù]Ø"keÀ<²Ÿô&­ê@`À"…b@4:<;ðq?Ñ+ºûéñ?Å¥o±"‹?ñÿPÈooú@	û2:å¯?ïË^£#†¿Ó0¿P‡Î¿çšß¿Ø¿çkº=©î¿ïøô=Te¿ï;f›ÖAGNfsrqPKS 0220-349?ïô'aÛ¬?Püî2b$Ñ?WÎÚýØ_?Püî2b$Ñ?ïà®·h•?y"Á†ú°ã?oQÿ9y"ø?y"Á†ú°ã?ï—òO	ÊÑ?|ýu•½à?Šl@üç ?|ýu•½à?ï»üäO?g`d[ä?ûø'P:?g`d[ä?ïécŽù5>?`>7&"Š­?fœpç.Yþ?`>7&"Š­?ï'õ"Àg?"S03Œ?x¨ÎV??"S03Œ?îÂTfÈ|?—ªâ?K²?£Ú¹¢ãC?—ªâ?K²?î'mÂÙ·?'Lh ò?§Þi"ö}Š?'Lh òAGN4FGL J0223.0+6821?èm
îïÑ#@ïÏ_ND1À9ë¼&Œ[ÃÀ<Ê<ϔ'@ —W´?þÉÎeS@ð?¾¨*+!ÁÇ?¹Fho*/S?ûàÇ¯;@E®CÊ°¿á€À_+3µ?¬–ÄŸÊ®¿ã.Ò{bw¿Ô.iàCw#¿âúã±à¿á6YSXmAGNbll3FGL J0223.3+6820NVSS J022304+682154?ïûòR?9Ó.ᙥ?CÇÅ2mö1?9Ó.ᙥ?ïßÙ —?qÚPìÎ?pp?ˆƒ?qÚPìÎ?ïðÄ=(¡×?W8áüg?^w†	r>?W8áüg?ﵤUp†?böGšËTF?'–ê¬uƒ)?böGšËTF?ïïüIª?W8P
¿rP?`ïÞÒÍß?W8P
¿rP?ïF=lz°(?¨Ûjš3»?—8RraÈý?¨Ûjš3»?ï؇ÎèJ?€rt§÷Ê4?s¼t­)ƒ?€rt§÷Ê4?îl¼Væ?ÿ$ÄͨT?§)>3^ªš?ÿ$ÄͨTAGN4FGL J0223.1-1117?Ú ¤).f_ÀO¡Ò|96'À:6–•[À<}Hé}Ý{@ f&áÁ&?û*|«LI…?Ëkûf=K»?ª×Äøm?üàÝ%	¤Ä@\PÈðIT?îI=@}H«¿Þ•ØCùT¿åµmÕÆp'¿ ûsÿ+CÑ¿ás~§Ð¿¿æb»K›	AGNbll3FGL J0222.9-11171RXS J022314.6-111741?ïÿXÉ«ì>?ÎTú(Ó?æ̦ÒC?ÎTú(Ó?ïô#4Úʉ?ZŸh¹È{>?W¹–Î[íº?ZŸh¹È{>?ïöL\œZŒ?]LºÆ†Ó?SgFˆE?]LºÆ†Ó?ïúåÞZ'œ?+³úZk™X?Dh…©pE?+³úZk™X?ïÿEt&T?ûÖ{ Ý?\ò.¦@Z?ûÖ{ Ý?ïÙÄ õ?uª
¸Ãn?sü½oՃ?uª
¸Ãn?ïò¤qÑÿ?e¢¿ë?Z·ÖÒ$qš?e¢¿ë?ïò9óR?L…@ìÃ
×?Zŋ¹&êµ?L…@ìÃ
×AGN4FGL J0223.2-1653¿î \ë#¶$ÀPœ!ÿ.HéÀ:¡'&цÀ<,:ñm–@aĪêNé@(Fya?ÑéQò;?Ûbs'žÔ@	¬s@i|›@	("ÌUX¢?ëÚ7ïZ–O¿Ù1¥^ɹó¿ê"÷€Õ}u¿í+LŸjéÙ¿ïý—ÛSxM¿Ãˆ´oõ˜AGNfsrqPKS 0221-171?ïËîÍÊð÷?"ø 5 :Œ?z™+µp?"ø 5 :Œ?ヤ¢†I¨?ŒlÑ""Ö?€Z×Tή
?ŒlÑ""Ö?îÅ‹R•4?"¹^v|	ñ?£®gIÞ¼?"¹^v|	ñ?ïˆI2#Õ?r0.†b?í³zªæÕ?r0.†b?ïÂ'2ÛÚ?‰´C¬½ø?~ìf–ï?‰´C¬½ø?íN	½?½¢'ƒbܪ?³U H?½¢'ƒbܪ?íKd'hâ[?¥YZ¯æò?µ¤Ût¸í%?¥YZ¯æò?苠ðP	®?³Ä¥ÕÊÉÔ?ÍÑ|>¿ÙI?³Ä¥ÕÊÉÔAGN4FGL J0223.5+5415¿ÛD`™À'oÀêÁ5¿ÕÀ;UZ'ÇÆÀ< ×Ê,ß@!níËuì?ú½ý¬h©7?Øy*"é9?âD Á@§@=\œ¹Ë@}µ…]w¿ïä…CÛ¿ïÿêњ'ç?ð?Æ´ž˜1Á¿â¼œW~¿æ¤À>IëAGNbcuGB6 J0223+5413?ïþö€$}Ž?^Á¥i? —ù‹muó?^Á¥i?ïí}õµ`?hü¥¾ÿ!c?b€ôM ›?hü¥¾ÿ!c?ïÀÄ	
¿?yݹ)­?û'UØ"?yݹ)­?ïÙŽØÂÇ?bÌbÕÉ[å?sp¸qòpÖ?bÌbÕÉ[å?ïþ;Hš<q?6è#`·Ô?,Kto¤-?6è#`·Ô?ïž £ä®?"H,§ng"?ˆw×-øš?"H,§ng"?ï¿_±–eˆ?"à‰¿>‰?€(¦Å6	?"à‰¿>‰?ïŒfX?…wqÏÆ¿Q?Œà&\:\€?…wqÏÆ¿QAGN4FGL J0223.5+3912¿íVÔc«1XÀ4BÁ HàDÀ:†câ'§åÀ<yˆ¥U@²Š}òÊ@¾4[Q_n?ÃGÃx4–?¼b	4‡=?ö®…ÙÚ@¶œ€SÍ]¿ÕÜrÝGÅ¿á‡gÓMðN¿år5a¶©J¿àyêaÞv¿ÞD]·ì¿ïíE]'<0AGNbcuB3 0220+390?ïý‡Ìg8?$ü?4¸?3Á~fNO?$ü?4¸?ïô-SË.<?W¯\˜ 5?W¥X,è"?W¯\˜ 5?ïñÿu\?q¨Õ…ÝÂ?\ᇁ?q¨Õ…ÝÂ?ïòDO²'0?=ü÷è•×¼?[w`w¯e?=ü÷è•×¼?ïüÑJÇ	Ð?1Ϊ3Ç-?9u¨Ie?1Ϊ3Ç-?ïÏKÕkÙ?Þhe '?xZ<€£y?Þhe '?ï鞥Ù)8?vûk™
‰?faZ;tp ?vûk™
‰?ï¸å>*)—?m˜3шZA?Æ°|¬ÈN?m˜3шZAAGN4FGL J0223.5-0928¿ån>LjWÀNÿ‰?¯BxÀ:ã‹+AÍ*À<¥­ç.wã@$£ÞlŽ@×:ÿ°Nè?Ì
,"óŸõ?Í4M¦‹ð@ð÷"0{É@(Ätñ¿ïÿÞ!ˆæÄ?ïÿíáoq'¿ããªÿójÆ¿áTî~ù/V¿é¼êº:#¿ïö…Î
ºnAGNbcuPMN J0223-0925?ïëÙÜê?`|éyǒ^?d&$a6?`|éyǒ^?ïÞy[qÑæ?~‹¶[?pÃR;ha??~‹¶[?ï]`·aø?'ë̞'¬?"Séþ©?'ë̞'¬?ïǍ"Æ\#?a(¥E^Uä?|9n«ð6q?a(¥E^Uä?ﷸȫLl?z'tk³?'ÍÝþý?z'tk³?ï'Úñ'Êõ?˜4¥N?‹‰C¤ß6Ì?˜4¥N?íp"_õI?¥lò†?«¯?´{]U¹?¥lò†?«¯?ÃË-?"Ú
fÐ"?¥.çá/˜:?"Ú
fÐ"AGN4FGL J0224.0-7941¿ëtrúÀBAþûôÅÀ:liÁd¹¾À<|Jù"–-@J&>Ù@%Û[ÛÉ?¹Û©´nÝ¿™1¿ìÞ?àæzÕéV@Læ/ŸTï?í"Þ9Û¿ä©Q†¿å
$¡u;¿å¤=ÔÌË¿Óþ_o×(¿çˈ>¨\UAGNbll3FGL J0224.1-7941PMN J0223-7940?ïý"éA«$?&ÕÚ!6©—?6è·¨Aì«?&ÕÚ!6©—?ïö«Vk­´?T0·Óúg2?R©SZ÷=?T0·Óúg2?ïõkŠp9'?[ñ™Ú¥ø?U(êž[­ ?[ñ™Ú¥ø?ïü²Š£©à?#XH–=?:k©ºì9³?#XH–=?ïùQxÿ¬Y?B¼Eы?Jº]Ãî?B¼Eы?ïÚÄý†º?~´X´?rðŒ;bÜ?~´X´?ïò\ÜNõÜ?j/2*8?[FG–NVì?j/2*8?ïñÖ§A"	?M¶ë¼Ž,?\R±#=ÿ?M¶ë¼Ž,AGN4FGL J0224.0-1850¿ËUûñ8ÎÀPËʖ'§]À:ÚlVjoàÀ<•?†'Í@ gšÅ=·F?ûµ1öQo?̩͜çD?ÑŖb,šé@)à¤&?úæîÄnYz¿¡%uŸ-F#¿ÚRÅ؈?çHšÙ4º¿ÉH‡r¥¿á•îê.¤¿ïÿªÛ
}2AGNbcu3FGL J0224.1-1846GALEXASC J022404.29-185029.9?ïùG|ڂ?>PÒöh¼ú?Jã¡Ãwà²?>PÒöh¼ú?ïÏB·Y?'튚À»"?xyÞ¹Äge?'튚À»"?ï¶Û	Œ¬Ý?x±gÐtå?'I=¥ÃĞ?x±gÐtå?ïDà7ôÊ(?}
Ψ€¥t?—cùfºþ?}
Ψ€¥t?ïõpj?Pœ+SǦ"?Uç"Å?Pœ+SǦ"?ïtMDßá…?™‰+›
ô*?'vWi+9U?™‰+›
ô*?ïk»›)Å)?Žvà÷|#?'ˆŒ—W¾ç?Žvà÷|#?í¡d§}©?¢ÜqÊ6‰C?²ôÚÄ'º?¢ÜqÊ6‰CAGN4FGL J0224.2+0700¿ê~|¨.ÀH'$cŒ—SÀ:wpoÔ¤2À<F'ŸªTÓ@Rý8$‰¢@êN7›wÀ?Âc\›·V?±áÁ'ýö?îí{ì	©@«ºCf§?À®|ª }¿âÁŠÿ¢âî¿æ'~Ý«—¿ëÙ—Œy ¿Ê
#D}³_¿ïþËí©¼'AGNfsrqPKS 0221+067?ïþÖ;OP9?}tō'Î?"œG&ÔY?}tō'Î?ïôp"™Ï—?[®]á?Wöâ^RE?[®]á?ïò`Ç.ìì?N<G½$Ð?[>q"g·'?N<G½$Ð?ïþG
…¤š?_ØÖkÉê?+*²]™9?_ØÖkÉê?ïþ€KiàÄ?$4­ÉÈaC?'ûGá}?$4­ÉÈaC?ïÖ
&?k?zJyGöy?tùlã
*k?zJyGöy?ïðÃ¥uŠ?c4ÿ‡ÜÊ?_Ôx·Ôœ•?c4ÿ‡ÜÊ?ïõí›_©?KS~êX.X?Uð$ÈÏ3?KS~êX.XAGN4FGL J0224.2+1616¿ä±Y÷ ÀDü;OagÀ:y–JYÀfÀ<J¶4‹@²($·Dz@jlBHyì?Á=z^ëÈ»?©ËndÁ˜?ê´¯ÕEAS@xƒÚ?ï;2G¿ÍEäßq¿æóÇb¦ÿ¿á"Þt"ý¿ÞÆlÊS¿àÅFÞ	5AGNbcu3FGL J0224.4+1615NVSS J022411+161500?ïú¡;"?a
ÃLûA9?E{ŽÛ¢?a
ÃLûA9?ïôE8æÑ?X²àöy\?WuŽ=Ö?X²àöy\?ïÝÚ"·m?~ž?ªg®?qî÷ô]ª?~ž?ªg®?ïïîQ¤.ë?@ÉG}Bá?`®8$ê?@ÉG}Bá?ï÷"ûúÚ?FFà)¹?QºÍÒ¤ß?FFà)¹?ïќ‡à‰˜?w<|ç>	?w1¼LØ?w<|ç>	?ïèþT6ì"?uiÇ`#›®?g«Õr?uiÇ`#›®?ï±IQé½Ú?o
°¯Dö?ƒ­«"¦ïM?o
°¯DöAGN4FGL J0224.9+1843?áǾ":ŸÀCn¾H¥‹À:ìxc¾ìÀ<	haQT@wv./"@CEÏíé?Ç`ü" c7?Õ½½eP½@i¬ÿ§ël@¤yÊl˜¿Óp¦{RF¿çF—ɵÁ¿ì¯D]f¿ïÿÿ&¦³?ïÌ"'áÇ0?ìMÃ\á'AGNfsrqTXS 0222+185?ïé(¦Îq¤?¨3ã%aŠö?f×Yn{ê?¨3ã%aŠö?ïöa. ØE?USŒ¯ÿI?S=£ÑE2?USŒ¯ÿI?îõm¢<M?Ô×ëáPm?¨©(oð/?Ô×ëáPm?ïÿõòÇ">ÔQkdRþW>ÔKƒÆ>>ÔQkdRþW?ïþûÈ¡D?,ï… ð? O‡%MG0?,ï… ð?ïÒD퉟•?€¥H'èg?v݉B¿YP?€¥H'èg?îh­|ê%<?F4	x?©u(.É÷B?F4	x?ïþýNÓU[?"랠¦P? +º»7r?"랠¦PAGN4FGL J0225.1-2604¿Éùj´¸óÀQCÙ+à‹À9xöžWn|À<oKG&/?@f,êįr@ÚÖzËx9?¬¯àš?°ˆ©¡x—?üâqÊG·O@,æyq0¿ÒvÊÍL'¿ã™_÷·\¿æúK '\9¿æ˜§8Ϫ¿ì÷Î8׋¿ïþÊ@*'{AGNbcu3FGL J0225.2-2602PMN J0225-2603?ïýە	Š?"Ü˂/±…?1#X]Âk?"Ü˂/±…?ïöYÍj›C?TÝj?SLe'¿y.?TÝj?ïë";¥XÑ?X,ü_Öb?dÝÄNH—Y?X,ü_Öb?ïÿK{Ã3¶?%t©^E?')þá?%t©^E?ïþ÷¼åy?2Œ»L+|? "-ÂW6?2Œ»L+|?ïÚ,e}w?vp÷¯éƒ?réÍM£t?vp÷¯éƒ?ïïJÆÖFQ?cpðV@?`µ9!zŸ<?cpðV@?ïþ¢|"î?Вvcã?%Ø?Ûÿ
>?ВvcãAGN4FGL J0225.6-4502?ÚÐ%æÞ4ÃÀPNe¾ ºÀ:ËY%5C¯À<niØá®@Ú}¬Þ@ÓÁÛØ‹?ÁÛ«¢Z³U¿`7hÆÕ]?'Ã`Áû@á9|Î\Å?ëÅ3 ïò¿Úˆ€Âˆ%¿èri>‡û¿â?–ƒd£ï¿ë}·PcÅ¢¿å۞¡Á0aAGNbcuPMN J0225-4503?ïþ5ˆ€ ,? —ƒ|å?,§zYQUq? —ƒ|å?ï÷ßìº(?Vh¥JǸ]?Qâ@,ï?Vh¥JǸ]?ïÎ*Æ/Ø?€Â`;cŠ?xðj½äS³?€Â`;cŠ?ïþõ>ŽŽ¬?	éû
‰á? ¬n€Äô?	éû
‰á?ïýØ8÷Ôt?)ýÄ[‰¯?1>9iԋ?)ýÄ[‰¯?ïÝäh¹–©?tiô/#C{?q
ː¦Ç¦?tiô/#C{?ïÚ(âÑ?{!ύcVÅ?rÀkäS»?{!ύcVÅ?ïüÏgŠ?+@Ë6X>?9"ÆOµs?+@Ë6X>AGN4FGL J0225.8+1310?•÷ƒu9ÒÀEÑ¢Æi}À:NÈ.›À<Rû15,@ü'Ñ*T'@üÛ`
†Ñ?Ã7²žÎ6Ú?¿0°Ìæøó?úÆ&Nyá@Ú_‡z¿³ùû€Q¿æ(¾e*ý¿ß=ïN×Ôh¿Þ°JJ¦í?¿âqâE"ï¿ïÿm²æAGNbcuNVSS J022551+131046?ïýî•óª?#u¥uÿ6[?0‹V4¶'~?#u¥uÿ6[?ïõ=¥ºX?W1q-¾ûæ?U"¶QAr?W1q-¾ûæ?ïô4^Úß?]¼ãuÅ9?W—Ûœÿð³?]¼ãuÅ9?ï÷]Œ ²?3ºÐMR?QDèøªù?3ºÐMR?ïû+*-ً?>¡V'ŸO?CSX6ç?>¡V'ŸO?ïÓتP¡?x{ö°rç?vªÓöä?x{ö°rç?ïð¥õÑŸ?i("+ð¡?^´ý¿²(?i("+ð¡?ïÝ[E(Ë?^GÔiG?qRuëÙö3?^GÔiGAGN4FGL J0226.3-1845¿â{ìo ìÀPª¼£nÀ:¨"7blÝÀ<l¥Ö¾¾@ p®øU@¡Ðº˜ã?ËÇrÅÅFœ?ÉAóU?ù¿g¤T¿@¬äúëï?ïÊBy!T¿àâՂ}ô"¿é\sÔ
2î¿è=•ø$il¿ïþÁ¦þÜê?ïñ"aÎüþAGNbcuPKS 0224-189?ïÒBwÉ»?¨@8d¬o8?vÞÄ"¨9?¨@8d¬o8?ïõ,Ý'?Wkf­È?TߧJ}@ä?Wkf­È?ïžHCKëL?†'~À'fP?ˆmï"¶Y?†'~À'fP?ïýúZ[Ó?IPtТ?0-2—¶3?IPtТ?ïû4g¡à÷?HY!Ë{Ï?C.aÞ½P
?HY!Ë{Ï?ïØÜð'è?uú7TC¼?s'‡ùu?uú7TC¼?ïXõé6öó?Ñ$Ú±»?"áBá¸'Š?Ñ$Ú±»?ïõxÄ¥?I™â}?U1~×9?I™â}AGN4FGL J0226.5+0938?×kZLãĜÀGMÔ{í·(À:lôI:ÜÀ<a&õ7O"@<«S«MÌ@Yúb1M€?Æ06(°ù?¾ÑGA_Y?úß;ÒDÜ@"˜ÒtV"¿çØ÷°Õu?èά5}O¿ç›©¿+¤t¿Ê,Æ`¢¿ètõ_èóÊ¿ä{aT¯AGNfsrq3FGL J0226.3+0941NVSS J022634+093843?ïÿ@q¬	?
¤RŽ¤/Ò?ñÍ«gh?
¤RŽ¤/Ò?ï÷4"è÷?T'ÞC¦»?Q—õN$	?T'ÞC¦»?ïîêî9Ƚ?jêeC»"'?a´YJ¶?jêeC»"'?ïÿæœgæ?1}‡1À?£%¶úqÿ?1}‡1À?ïþ$ï´¿v?.'¿êé{Û?-±ØÍõ?.'¿êé{Û?ïÎ|Þ´%?'êÛõ"¾?xÁ«vÍO?'êÛõ"¾?ïÓؙ¬y?9‹DGÔ¿?v³=;6?9‹DGÔ¿?ïýͼŸ£?)1?bk¨8?1' E'Ã1?)1?bk¨8AGN4FGL J0226.5-4441¿Ûã2¼ìÀP6Þ¹^[À:_Í¥òmÀ<uW¿Úv@ Xûâäç ?ü̏	óžÉ?Áçt†B$?Á0ŸD©RI?ý0 Y;Û@5qß@lØ?Ó_JrÉK¿êС£SV¿¿Ãz
?åH¿ßœ{¡6¿à7#"ú¿äÚséܨAGNbll3FGL J0226.5-4442RBS 0318?ïÿ7¸Óñ"?
¥0BMû?è<8`4?
¥0BMû?ï÷?k7Ô?UƊˆÅ?QÉcIÈ?UƊˆÅ?ïø{=|Ñü?[£Ü"ôò?N
)Ng…?[£Ü"ôò?ïüü›ØŸO?"ˆR€¹
ð?8"¡v^?"ˆR€¹
ð?ïþb×Vi?$žOîß¾ ?)Þ%6~æ?$žOîß¾ ?ïÛYŽÖ`ä?s`Ø¡Y	?rS8z²†?s`Ø¡Y	?ïõ—¢Ò?eöe5…'.?TüÐÕØՓ?eöe5…'.?ïøÐX>ý¹??.¤!.%¬?L¾žRvæ??.¤!.%¬AGN4FGL J0226.6-0553¿ÓSŽ¿ÃÀMz
í(ŒçÀ:t`§	Ä¥À<—À{†@ÕüT#î@ä;ÜO Ð?»¹J9	6
?'p%_"—?Ôî16ñL@¥$Yт"¿´¡¢¿å0¤ãy·|¿Þ'Ðý‰H¿åÜv"œ;¿âÇîvjÀh¿ä§­­"AGNbcuPMN J0226-0552?ïþ zÚøÆ?!O8öÒ¯Q?-øO‡÷Û¼?!O8öÒ¯Q?ïõ«ñ¾|[?X,â!úÑð?T¨>O?X,â!úÑð?ïôw]{þv?[Òpo
³?WECdò?[Òpo
³?ïý¤å
q"?%jB6rP?2Øؾkj?%jB6rP?ïü?k·?6Ë0‹?>îAá†~?6Ë0‹?ï×!"½Pr?ñ©ËÌäÎ?to6:¿>?ñ©ËÌäÎ?ï÷DÝ!%6?añÚb^‡[?QvF+©D?añÚb^‡[?ïù,ìXj?=ƒ:Ì(á?KóKvÇÒ?=ƒ:Ì(áAGN4FGL J0226.7+2312?à:Qïz»wÀAS¹bŒ½À:´ƒ*ÂKÀ<aÝ6§[ú@ 6՝@YbÝDê?Â˅úÖJz?—‹|ËW¬º?ÖÏ;üZ"?üà/€ L¿ïRW…øÒå?ïÚî}÷|¤¿ãϱƒ›*"¿äŒé‡îvk¿æãÕAæT]?À‹#õ}›AGNbcuGB6 J0226+2311?ïý­/M r?%¤ZÀž—?2–…}ˆ?%¤ZÀž—?ïðÀtÐ?`º
h¾ÏA?_è€Ώ?`º
h¾ÏA?ïêvøž¦Ž?am*®\þ?e‰6¾J®?am*®\þ?ïÕuU #)?ZðÛ/û×?uEU+Îão?ZðÛ/û×?ïøÿÉào}?CxpýUèJ?L×¼¾rì?CxpýUèJ?ï¾
ù>?uà²$?€}A 9–?uà²$?ïàµv]Ä?wtbdd?oÿJlń?wtbdd?ïôEjK?ŽªæA>Ä?žwPþÒ?ŽªæA>ÄAGN4FGL J0227.2+3928¿á!‹gôËÀ3Áޜ)¦À:Qnf)À<
ÏCŸ'@Ê·Í·-~@ÿëJ?ÄúPþöÅ?£"$à_%Õ?ØzšÛ@
ÈcCqCå¿à«RÿU¿ær»ß>¿X¿ê_«+'U¿âÄC@Çpl¿ïɧ~^ª°¿ïâÁ*ØßAGNfsrq1FGL J0226.0+3922B2 0224+39?ïý3_(ª?/W•AÖ=?6e*ZÁ?/W•AÖ=?ï÷ÖàÄGå?Oq~u$Ø^?PR>ƒˆn¶?Oq~u$Ø^?ïãgS cx?ph"dÁ5?l˜¬æ{À-?ph"dÁ5?ïûžtl0?/tµ%L5Œ?C¥†KrVd?/tµ%L5Œ?ïýÕ3VLF?2ì²I'Û?1Vc:iá?2ì²I'Û?ïÚåUý?t°ó¡!¡.?rUÛK?t°ó¡!¡.?ïÒ¢;v0?|ü°Þeó?v®â"–Ð3?|ü°Þeó?ïã!ç¶6?`ùŠY–?lÞå*Aí?`ùŠY–AGN4FGL J0227.3+0201¿É!hì§wÀJgãŸw),À9­ÑI3O¹À<,Y4©@îÞA>c¾?þÈ;4¦?²D
Ëð"??œÃD¹?ì¤ò'Ð(¢@4>=¨W"¿á¢žA-¿àÂñLO¿àŸÍàÉ¿ØKêd7b¿á‡Û+4a1¿Þ`ø=hì(AGNbll3FGL J0227.2+0201RX J0227.2+0201?ïü;ÂÎÇ#?0—…þ*¯ô?>!è9Sì?0—…þ*¯ô?ïôl6ñ?ZðÝȨ?W''L'˜?ZðÝȨ?ïíÌÔ¯oD?g{s…Ç'?b3+SPl"?g{s…Ç'?ïóäï‹ò?D.n6à?X6 ›$Œé?D.n6à?ïõswÏx?J"ÆæàW&?Uû[£?J"ÆæàW&?ïÓíni%o?xi雗")?v	HÙ+¸'?xi雗")?ïëœàdÈñ?qý5
ëˆt?dcޏfi?qý5
ëˆt?ïÙØœt?cåu–TG¯?sý|±Æ%?cåu–TG¯AGN4FGL J0227.8+2246?눕']q1ÀAvÐâ2À:'3"«CÀ<S¯s²M@ïæÌRT?ÿI-U£ "?Ï0šgó
?Ë›Â߁@kq'úä@kÓ}–á¿è‹ïŒë5n¿Öa/šÍKM¿á‹öþÏ~X¿ßØxýlÒ¼¿æѳ¼ZŽÂ¿ïþû=x†zAGNbcu3FGL J0228.0+2248NVSS J022744+224834?ïýpòð?,¡¾D‹"?4xikígÿ?,¡¾D‹"?ïõyMì†?U$©'òÅy?U
d5—c?U$©'òÅy?ïåÄz˜Íl?cÉe@ô¥?j;…˜¬óâ?cÉe@ô¥?ïý[Á$€›?ä¼sfC?5!õ¯Ðy?ä¼sfC?ïþWzÔ÷-?)5?Ÿ[@Ò?*ˆRŸø,?)5?Ÿ[@Ò?ïÚ…`–]?sC~Ž2(¸?rñ½p±‰?sC~Ž2(¸?ïÀÍ?I¨?€j
QCë?û™yÈGÊ?€j
QCë?ï÷²ÅÿB?B¤YÃcb`?Pšsã?h•?B¤YÃcb`AGN4FGL J0228.0-3026?Å¢1BÃ"ÀQ'N;Í5¨À;óÜ܉À<·‹"- Ê@MϹ'0¿@î#yÌ?Í×¼w¯d?µ±-œ"`?çؘ²é̸@óÔyêQÃ?êDXŠÑ ¿Ûw"}~[¿ã*l»>¿â³_þÃ?¿åª""Žö(¿å0´hQøñAGNfsrqPKS 0225-306?ïÿsðN?Z­–ñE?ø´·¿Z?Z­–ñE?ïöô:qbe?Sõé|í?R‹£ëä¶?Sõé|í?ïø9lÞ$¹?@)ÈQJü­?OLêî˜{?@)ÈQJü­?ïþл¢`›?
eDÌy˜»?"ôE­ûM®?
eDÌy˜»?ïÿ¨¤ôE?wèÒ'?×8룀?wèÒ'?ïÛ/4º¶?j}À,N?rhe'Xdç?j}À,N?ïú"‹?Ž¶?R˜l
ó­?EíÓCFú?R˜l
ó­?ïýÔ4Ží?(ë1tÚu?7é\«lð?(ë1tÚuAGN4FGL J0228.1+8208?èÛ¸¶H­@3뚝¥—ÕÀ:¾R}{UâÀ<\±•+v@je›»1ð@" ß8´?Շ#	ðCÊ?¤k·^%¥+?¬ûŠûF1é@¥CWm¥¿ÖYì x±¿è¿¾ëbº¿ã؊:N¿Ý$þývÑ¿ïÿô╋î¿×·0ÃÂ7AGNbcu3FGL J0228.5+8213WN B0220.3+8153?ïþš×¡?&;­‰O!>?/FO¼k?&;­‰O!>?ïó²–b$?[aªÉӂM?YҚR
h¬?[aªÉӂM?ïÚ=*OVL?uǸñb«3?rájÁ§n0?uǸñb«3?ïýkk'|? °'ŽXë?4¤¤Ž².? °'ŽXë?ïþÁǾ£?%í•q*?#ãé"ä?%í•q*?ïÓhö"?}=T¹[¦þ?vxKyþ¯*?}=T¹[¦þ?ïßuæƒy"?}<éOBh?pE·cþ?}<éOBh?ï÷MuÃjg?AӜïö"?Qe?qÁÏ?AӜïö"AGN4FGL J0228.2-3102¿ï«º0ÀQ"gßã*À;C—'h$­À<Ӂ¶NG@tãÞaIÇ?þùúnƇ?Ï2·¸=žœ?Æ@b†2¼?÷š™ÄaÄ@?þ¯áa{¿ïŬý¤†?ëÊGÅwÄ¿Ô
=¥ýÖ¿êQÎ(í_?µÿjXäG¾¿ï÷£:,K¸AGNbcu3FGL J0228.7-3106PMN J0228-3102?ïýØ@{ù©?,#SXÆ!¦?1=üʟU°?,#SXÆ!¦?ïò®¶aP}?dÅ"iŸ?Z¢"aõî?dÅ"iŸ?ïÎ`ÀV".?rkGY'h«?xϟísý?rkGY'h«?ïù%+ªö?:µŸÿ¾šÖ?Kƒle½U?:µŸÿ¾šÖ?ïùT·K™?F"î~Q?J­#5ó?F"î~Q?ïµ1Cޕç?RðR—?'³¯'ôR?RðR—?ïŽ?ó	?‡&ñöÑ#?Œp:u}ͺ?‡&ñöÑ#?ïÒI˜Uç?qZEomš'?vÛq®U¬È?qZEomš'AGN4FGL J0228.3-5547¿Íp¸
.=fÀL9BÜôb=À8$_Ñ÷®ùÀ;c¤¡4˜Ž@Z4!š¯n@κ'®š³?zùà V?¼âW–>ñ@!±>›A:@€yMHÞ?ë°*Öm_¿ÛœEE"o¿ãZ¡Ëi¿ä!»qZ¶/¿é1ÿ×f.¿ïÿ{uÂ#üAGNfsrq3FGL J0228.3-5545PKS 0226-559?ïé¤aÒ#?be6£p¬?f[ŸéÌÖ?be6£p¬?ïî¥!4?n\'ÏîcÏ?aZëè³z?n\'ÏîcÏ?íå®;xbN?¢X^Þ)7ÿ?°ÒŽ"…–?¢X^Þ)7ÿ?ïû'ß¸?@"ë–~	Ó?Aù´jƒ4S?@"ë–~	Ó?ï'ÚÞ2zÒ?ƒùã*$?‹IH}°'?ƒùã*$?ïÊÞ6<ä?"ËT!¡W¬?zäÓρz?"ËT!¡W¬?îq^ÉRގ?žÝvUVO–?¨êk­þ?žÝvUVO–?ïåò"†%ã?dºÉ¯îŒ?j
{Y|Ë?dºÉ¯îŒAGN4FGL J0228.5-2234?ç¾Ì¿$²ÀPã8`™ËÀ;i+Õpà=À<ÎÀMb‰b@")øL‹@Ægeiç$?ÓsšvL?ɵ˜RÇ£?õàèÄ3¡@+ˆª&À?ïÿ-½R†`¿à÷
}—"¿à8ÝA90M¿äesâ¥Ò¿éµ_B…¶Ž¿ïôó'H¡AGNbcuNVSS J022832-223350?ïïVñ?`H&UÆXY?`bë€Ã¿?`H&UÆXY?ïñ‰m…=?[Ï`'?vñ?\í%Df…?[Ï`'?vñ?ï¸Ø֒À¯?yMӕY?ÉÊgVv:?yMӕY?ïï¼îÞD™?C«

z0ä?`CðAã?C«

z0ä?ïà–¨Dú}?k>*@D
•?oiW°¹?k>*@D
•?ïÌx›"'ì?|Õ?º»ŠS?yòV²ÉÖ?|Õ?º»ŠS?î³áý>7Q?˜¨7tÿ?¤Áà,Šó?˜¨7tÿ?﵎a›ë?nÊäÛXv$?'»œX"ÇN?nÊäÛXv$AGN4FGL J0228.7+6718?ïoߓùǂ@Ã2Ál"À9´€JœÜÀ;€R'KÖ@WFbåÓ@j_ºzº±?À$Ù~6Þ?Ê-_Ÿ!î½@	ýfe§@zâ¾%À?ÎÈ2É«Û¿Ý7‹òç鉿é˜#wÔLô¿æ$Ç_¥'¿êaš#Ø¿ïÿ˒:)ÇAGNfsrq4C +67.05?îy8ÔÃøN?ªË7TǨ?¨lr´œb?ªË7TǨ?î؜é|¨??¡ük÷)?¢v1gY•?¡ük÷)?ï5¢û[ð?Žw¥ÉN?™_$åÿ?Žw¥ÉN?î‰ÙÔáÝð?€öaûÛs¨?§bb®r…?€öaûÛs¨?ÚÀùˆQ]?Í &ñÈÛ?⟃;ðWR?Í &ñÈÛ?ãÍó¾u"?ÐCŒÇ¤?ØẽÙ?ÐCŒÇ¤?âÁQ
[)¿?À0Ÿb¹ç?Ú}]åI¬ƒ?À0Ÿb¹ç?â'ýŸþbœ?³Dæ6ÞÁõ?Û°À:È?³Dæ6ÞÁõMIXED4FGL J0229.5-3644?܌CMeA+ÀPÊW)²€ñÀ9/»£¯À<TPâp£@gHûF‡Ï@´ž¢íÖ2?ªý¼¿õŠ?ÀuýG¾Ûs@ݺӦâ@[¥…`&±¿×GÝyÃ:}¿ãº{&Á¿èkZâ#Ì
¿ê>šš¿ïÿö?ŒÝÉ?ïþüà:è´AGNfsrq3FGL J0229.3-3643PKS 0227-369?ïù
Þ*m<?XÕy)óª˜?KԈay{¤?XÕy)óª˜?ïõ`ë/ìà?W·ŠýëÄÝ?U>)^-¿Ï?W·ŠýëÄÝ?îéæ_è?f?˜H+­­Õ?¡ašnj"?˜H+­­Õ?ïÿ"
¢V"?%ù`<?â?ýJ$m
$?%ù`<?â?ïúØ­øî‹?H!þ
(†£?DI"›n?H!þ
(†£?ïÖ'ÕmA?z$Öí@Än?tókôMë?z$Öí@Än?ïZHN+Õ?",Q+f—+?"¶ö5v»e?",Q+f—+?ïý«'áW…?-ÖÂé@?2£ê¹*ë?-ÖÂé@AGN4FGL J0230.8+4032¿Ôӆ8Ø}tÀ2€V>Ðö'À9^9ßõž}À;õp­è7@Owbâù4@r9`sÞ?²uFþí|?Áÿ_C}X@
ÔF"ú@´Â%~ê—?íY!…Æ~¿áò•S¹»¿æ­GÌGl¿ç$L£2¿êӆŁ~ñ¿áÉO?ÙAGNfsrq3FGL J0230.8+4032B3 0227+403?ïúÏ¿pmÑ?>HÝÁ§âˆ?DÁJ1I$?>HÝÁ§âˆ?ïõ™'$ï½?XS7×Õ?TÌݝcUu?XS7×Õ?ïÅÝ2(NÜ?x>+MMs ?}fܺIø?x>+MMs ?ïþ~$>Š?s½­'(?(!Ì:µ«?s½­'(?ïóïOrrÓ?Q¥~f!Æô?X!`ÛáŠn?Q¥~f!Æô?ïϑ{p—J?{Ë/·}X9?x7BUrʹ?{Ë/·}X9?ïsi|Êè?,´Êê¢à?''Ýk?9?,´Êê¢à?ïûøOm·¥?0ºO$Þ?@Âf½Š?0ºO$ÞAGN4FGL J0231.2-5754¿êÃøvZ
ŸÀKJGìþ›|À:ˆ׊•ñÀ<›Î ‰ãC@ ÀWH'>?ÿf[~«Ø?¹hgGŒÜr?wôMcS?Á*±"qê(@@œ5UL¿è1}ˆ¿ÔÔBÃI¿áÌoD[y£¿Ú[h¢×0¿áf¢vb¿ÙK¯RiAGNbll3FGL J0230.6-5757PKS 0229-581?ïþtí'À?*2¨ƒ}?(±(->j£?*2¨ƒ}?ï÷v7Ùyó?R'öAx5ë?Qì×
<?R'öAx5ë?ïø3FÃ!Â?T›ŸV' æ?O2åVm·I?T›ŸV' æ?ïþD†CÝ?¼öÜYb!?+·Ÿ³}¼ê?¼öÜYb!?ïý!ÆÏ1×?/D–­›ò?6ñÉ˶5/?/D–­›ò?ïÞ°|+–ÿ?rž—,°L?p§ÁìDD|?rž—,°L?ïû^C"cÜ?IeÔh$óÜ?B†ñÈn*?IeÔh$óÜ?ïû8àõ?6³,»¥Ç?Cóƒ^/?6³,»¥ÇAGN4FGL J0231.2-4745¿çu}ÒáÀNÑ}àÖo
À9¼<ÛR¡ŽÀ<wš‡Ö"·@W´.o˜@(0 ±»Ï?°sHÞ&wŸ¿—ápa«°a?×·ç"
›õ@LJڪ[¿ßnÑ"2w¿åhªC5ö¿êB€®I¿æhÈ@vÕ¿êæ°£¡Z¿ÍÆRIÎÖAGNfsrqPMN J0231-4746?ïý`¿?O¸H·?4ÿi8ò?O¸H·?ïööÈãwù?TôÊl+Â?Rn¯B¾?TôÊl+Â?ïÓRž™™Ö?|N­\­?vV°«£ñ-?|N­\­?ïÿgn¤"Š?`á0{lß?0è•ýÑ?`á0{lß?ïþ""¤½?*gÑc°˜?/×µ!aÒ?*gÑc°˜?ïÝw‰Q«?~rTL…¯?qD;—#~P?~rTL…¯?ïÐV7LÐò?€YNÃ
ý?wÔäOH³:?€YNÃ
ý?ïýʾ­	?+ð
@¹??1ª,0?+ð
@¹?AGN4FGL J0231.8+1322?ïøL8ÀE^Ž`€sXÀ9@¬ï·³`À;úØPŽÍ@?*^ù4µ@F1!àûX?¯¯4'àçÙ?ªØæ`œ¢ã?öÞ¿ù³?@ʚÒÔ£±?åaUðÍ]¿æ܁u¶e'¿ê±]À¥w¿á¾«¡Ú¿ínTqq\d¿ïù>JsAGNfsrq4C +13.14?ïÈQ<€k?´cΰ¢€»?{×a½=ša?´cΰ¢€»?ïö1"©¿Ï?V=$¢›{¿?Sœ÷´1·?V=$¢›{¿?ïÀ Øxã¨?'DÙ¼ßðÇ?ï"À$?'DÙ¼ßðÇ?ïÿ`Ùð²ì?cꞘg?ä¿¥ø݆?cꞘg?ïý Õ"0×?/vÝ|±*?2ùVnî+ý?/vÝ|±*?ïÖ?Òit?€!@*á)Ï?tà‰Î?€!@*á)Ï?ï'VœcÈ?ªzEÙ?‹ªXõÖ?ªzEÙ?ïþØòQµ?Ÿž!>Ê?"p߇µb?Ÿž!>ÊAGN4FGL J0232.5-1118¿ØØ&}ÿEÀN½u6
À;FϐÌk~À<³ãcGP@!#T33@?ø~ÃNžÊ?Ô—d54?ÑøXrÇ?ÿªœ"¤?@Î2eWó‡¿ïÓb³S?ïþ!†ù"¿Ò£*g¿Ç¨·aßC¿àMÛÀ…–­¿ä<×â)«JAGNbcuPMN J0232-1120?ïýùoíù˜?#°–¿ÙL?04€óRA?#°–¿ÙL?ïóyÄçûý?_{ñ߁>?Yu¹Õv,?_{ñ߁>?ïáD[­-~?hñ,›Æ?n»¤‹?hñ,›Æ?ïõ®ÒÞ+;??Ì¾Ô?T¢ZVçY??Ì¾Ô?ïþ=n[¹u?&\4é8F_?,)áÓ@×?&\4é8F_?ïÏÌ]*n?'´üe›‹?xÑS—q>?'´üe›‹?ïê)ÚD»?nÕü>\£?eÖ%ç÷DÍ?nÕü>\£?ïà¿:	ˆŒ?a«RˆöϤ?o@ÅÊ|sð?a«RˆöϤAGN4FGL J0232.8+2018¿á>Æ»LÀBIöã÷‹½À:S»'ˆÛÀ<Hö~vþd@!TƒêÛ«?üŽÛÐuÏ?¼"'¾¶´ˆ?'8W¾}÷?ɸ%õç?þªÿu@ž×?Þ"@œ¨AÓ?µê!ÇP0¿àÄ=ÝT¿Ô¡÷¡Œ­"¿ÚŠºÄ³¿Ìœþ¨çë6AGNbll3FGL J0232.8+20161ES 0229+200?ïüð.âÒ¯?(NÒ ƒ?8~Špס(?(NÒ ƒ?ïôeu$Å1?UôWpÎK?W57¦ì³?UôWpÎK?ïñ M+Ɯ?^‡¯ÙñQR?\¿fè'>?^‡¯ÙñQR?ïé®ö´8?Ma÷xl{?fQ	²?Ma÷xl{?ïù(¶éœÍ?>T…ƒg?K]$ÄÀ™Ð?>T…ƒg?ïÔ¨Ÿh?ta³*7¬­?u÷r#§û?ta³*7¬­?ïó"-/IU?fĤS–³ì?X×¥b4†z?fĤS–³ì?ï¼R$KJ?k:Êåï™
?€ëvô¼Ÿ•?k:Êåï™
AGN4FGL J0232.9+2608?ß<«¯æÀ?eO Ñ1À:ïj'"À<'Ù\'HC@ ¤¤ä%ƒó?ýí`Á
÷«?ÈÀ˜a
[ù?·è>˜A*?îï
'ær@=äÉás?î:¦>Ê.¿•+Êz`ª?ÁéýŠ.í~¿àœ~á\{׿ßµQ†'¿áhÖÏ)žAGNbll3FGL J0232.9+2606B2 0230+25?ïþj¸ì¸?¢V°Ö©?)T'Âït×?¢V°Ö©?ïód©Ö[J?\Y"¶÷Ž?Y6¬PíQ?\Y"¶÷Ž?ïóêl‰¯Û?C¶ô´æ?X+'WÔ™?C¶ô´æ?ïؾö{?Tx~‹àF?s "䐖Æ?Tx~‹àF?ïýŸzÚØ?,VŽšÝ*?3*úWÊ?,VŽšÝ*?ïÒ^Ø05Û?y RY‹Ûð?vГæ…:Q?y RY‹Ûð?ïô•yy?gk/I&ä?WñފÕ}–?gk/I&ä?ï'+d|¨?taäsB?‹u'
ã?taäsBAGN4FGL J0233.0+3740?îñá½'pæÀ4ñÁç–|¯À:ç±m˵vÀ<£¦Ç…ò@˜AÖd%D@‰cՒn?Ábǵá£É?ƒ:5ØeC?Ãþv½÷qç@'3úý?ïüp(‡Ç?"AØp!¯¿äÎZÁlœ`¿âü¯ég7¿ÜXRݦ)¿ÝDÉޅÜÎAGNbcuNVSS J023308+374201?ïþÆò˜8q?H
´Ø¤Ð?#Ø:ßΑ?H
´Ø¤Ð?ïõÙ;x¯?WZŸÒ?TM‰V¦?WZŸÒ?ïïò%÷¶Z?pmE,ùÀó?`
ÙَõÑ?pmE,ùÀó?ïüîÑbt?žýÿ1­Ì?8‰se¶'?žýÿ1­Ì?ïþõ ¼?೅0À? ¯8Ôë#Ú?೅0À?ïڋNbË?s7Ê⮸?rºxk\~‹?s7Ê⮸?ï𩕈?t®«–Ê›ë?_Ëþ_ݱZ?t®«–Ê›ë?ï÷ü"Xð?>©Ò;Ï8?P׏B5^?>©Ò;Ï8AGN4FGL J0233.5+0654?ç‡Y'à´ÀGøAþ¨,À9Ì$$¢v¸À<8 ŸGX"@þL'¸€@®ÓØYÈÉ?±.Ù\R;¿}éHi·dí?ljÂáçf@
GU6hG?ÄÜNŠ|›1¿ã>åD'׿äÉ)¿—>¿éú)Çy¦µ¿Ñ°Zü$ÿ¿Üw¹à`þHAGNbcu3FGL J0232.6+0646TXS 0230+067?ïþîˆ6ß?Ê{hçÝ£?!ÃGé?Ê{hçÝ£?ïõV‡‡YŒ?Xكl™â?URðp˜ ?Xكl™â?ïò¾<]?ju<¹`¿?Zƒõދ˜?ju<¹`¿?ïþò+
1?2zÖI? ÝDÈ"Qù?2zÖI?ïþ"tãú?øÒYì"ð?&¸µæ€]ˆ?øÒYì"ð?ïÚxtIÃ?vm'©7RÇ?rþCÚxƋ?vm'©7RÇ?ïꖩF­0?rº#Á=?eiVwZPk?rº#Á=?ïüТ¼¥Z?0W?Hp?9zìP'Ä?0W?HpAGN4FGL J0233.9+8041?±.@VZ M@2­‹`ñ²_À;X¯ð3íÀ<Ïoì÷å@"Ď_|½?ô'ß(#½?ÒÜëû?ÐÄ C?ùƒš¤["{@ªM¤x›?ïù9r•T¿èº'S¸¿ïbË#/°?ë©b>älQ¿à°Ã¢ÆO?Àš2›³¥4AGNbcu1RXS J023428.6+804341?ïùépF?C¾ÀÂJ ?HZ>`¹pÃ?C¾ÀÂJ ?ïî/½ Ì?d¨NÌïlí?aÐBü ¤?d¨NÌïlí?ï®r½ëõ?'ÔKÞõB?"cP§û@¯?'ÔKÞõB?ïòµ
¨t?M¬U'â€?Z•ê§š?M¬U'â€?ïôÁʸ\?UgÄLJ?V}δÆØ)?UgÄLJ?ï¹&ÔCþK?†~ŸZ]K?¶Jå	5?†~ŸZ]K?ï›\¶Jƒ?‡õÚu…É?‰(Ò_oH?‡õÚu…É?ïÌLtLØ÷?v¾.U©+ê?yÙÅÕsü²?v¾.U©+êAGN4FGL J0234.3-0628?³fviX­ÀM?À	oëÀ:š±§­YÀ<~Ûúg9Ë@ f'úÅÙi?ýN$Öyù?Á´-¼åN?±6ªy?ìÂ7åÒ?úÕAX:?ÐÑ`ûmt"?É
É݄*¿×—?!S¿Ûü›KŽ¿ÜÅ%Ä4ͽ¿éŠýtŠkAGNbll3FGL J0234.2-0629SDSS J023410.30-062825.7?ïü×#Þ¤?6•R‡y?9H]y8¨?6•R‡y?ïíD7M°H?hñÃӇ,¬?b»ÈÀ'ª?hñÃӇ,¬?ïìFãqÝq?nÊ/oùqú?c¹·]ß5?nÊ/oùqú?ïÐÈ÷Íxç?[ÜAؒ%Ð?w›"'ü£?[ÜAؒ%Ð?ïø~h¸?GKâ—R<?OÎ^¦íµ?GKâ—R<?ïÂëÀ‹~?…õŽŸÛ÷?~Š›TCt?…õŽŸÛ÷?ïé|)Ÿ?u˜²Çª?fƒñüÜü?u˜²Çª?ïXÔε‡?`6?"åf,Ìë?`6AGN4FGL J0235.6-2939?æI¢O9"ÀPÀØì•ÀÀ; ìy:~À<Ä(Ï,"ž@þ™&F|@~¡ñ?¸''™z¿¼'å XO¢@9µ/ê©@5¬(½c¿ÌéìjÕ·¿é8ÝA90M¿åÆ×ÀEÕͿب'n¯¶¿á ˜%ü¿¥ 6@Ù¹ðAGNbllPHL 1389?ïþ+ùÐ]?Ÿ`¬®ž?'
Bâ䘔?Ÿ`¬®ž?ïóî=¤•?W(XLü¾?X#"ûŽŒ?W(XLü¾?ïõœ¥ÎÂW?g(s÷k?TÆ´³X?g(s÷k?ïü…à\Õ!?*•Ý{óo?;Ðý\hó…?*•Ý{óo?ïý¤eFù?/¿£.¿‹?2ÜÔÁoQ{?/¿£.¿‹?ïÑ]`‹äƒ?vÍL\>?wQO·ýú™?vÍL\>?ïÞ_¡½?}6Õ<""+?pÐ/f¢±Ó?}6Õ<""+?ïÙØrƒ'?iÇüBn?s|"äúÇ+?iÇüBnAGN4FGL J0236.8-6136?ì…2Òú]ÀI¥`Z³«À9&u =)À<\·ã0¼`@âô©	Ï@ž~Û¨1ã?¥3£E"à?¢gÿÚ$?ôŒ]VlG@³O؀Š¿Ú{?¼X‹\¿à.¾#¼«¿çy!¿mh¹¿á ð¥ïé2¿è%ìIiÖ¿çêªcyAGNfsrq3FGL J0236.7-6136PKS 0235-618?ïÿ6Т£?	çà~²km??‰þë?	çà~²km?ï÷»Ów"?R£¿öm4­?P‰ú="÷S?R£¿öm4­?ïóè p€ú?dŠêlj?X.¿[w+z?dŠêlj?ïÿû9b>Á¤ÓlUPt>Ãȷr>Á¤ÓlUPt?ïÿmë¸AÈ?"ŒŽS´´?BÄö͍?"ŒŽS´´?ï×6@¿ôÞ?ƒÄnk̏?td߃ØÅ?ƒÄnk̏?ïïœÒÖsŒ?k	ë,/?`c-lä˗?k	ë,/?ïÿük‹ê>Éixµ-(>¿5ÀŽw>Éixµ-(AGN4FGL J0237.1-0714¿î‡DæA›‰ÀMY>_· À;«ïÌñÀ<×µ?èM\@!ÁŠN"
?ú-½qåö?ՔŒ¿kG?È`:Ó:¥?ó.a«ì@ÁÞtj
5?áîÜ÷½;_¿ËK|Öt+?Ö6¾£>^
?Ú7D9ë´¿ß•ë/³L¿Ù±ž6ò…AGNbcuSDSS J023700.77-071307.3?ïüÊ%¼?,̦_x.ñ?9®Ö`1ëS?,̦_x.ñ?ïó>ÿP3?\Á®3ûP?Y'@Òy#?\Á®3ûP?ïåÂôÞ?lÏ®s,]?j=éÃq:?lÏ®s,]?ïõ¶5 e?BDu|ŸÅ‹?Uæ"[Æÿ?BDu|ŸÅ‹?ïüìsA|]?/'ƒ·Y'?8œg¸LW?/'ƒ·Y'?ïÓóAM¹?uŠÎ%ÛG?v_l®sU?uŠÎ%ÛG?ïâû¿Bdm?qÕ¼àO»?m@''Jû?qÕ¼àO»?ïâ³QYA˜?d'váµ?mL®Ù˜Ÿ`?d'váµAGN4FGL J0237.3+2000¿îQm=p"þÀB,{5*"8À:úK‡½ÏÀ<x篷é@ [' NT@úŸ{Zê1?Ä×	&Db[¿v"ÞÖ¥ï?ªq)Ò?ÿÙ¨'{ïæ¿ê†_ô‡Q?¤¥b5æR¿æ;Z^›@ä¿ÚOõ^f¿ía@"ð'?ãT|YóAGNbllNVSS J023720+200033?ïú2ë(œE?>e¹Ë¤?G4Rck\Š?>e¹Ë¤?ïôÈO ¸X?WåÒâxv-?Vo`çʟ¹?WåÒâxv-?ﴇ‡¯r…?}©Qø@?'Þ4bÇ?}©Qø@?ïõO˜¢+l?AwK9¢|?U`ÎUô¸S?AwK9¢|?ïò"y–'I?WŸx£!O'?Z×
FPM¡?WŸx£!O'?ïÎg´µ§?€è¡_¥ÈÍ?xÌ%᧬'?€è¡_¥ÈÍ?ïÊl"#™?€íãWY¬d?zÉîꏛ‹?€íãWY¬d?ï¼>5V	]?u ¦2Ë?€ðr¤N\¼?u ¦2ËAGN4FGL J0237.6-3602¿æèïêÖo…ÀPq¬ÄÀ: mÉ17À<}Ötì;'@ ]€‰¨4è?ü²›É?¾a"ðg‡?¦_
ã™ÿ?ér\©NBƒ@
'r—Í?êíý¬i¿æ¯2BGx:¿¹ÐÔÄ=F¿Ü®}†¸–¿äú•þ¦~?M/]»œúAGNbll3FGL J0237.5-3603RBS 0334?ïÿIMô!?@ÝËN?ÖBð`9a?@ÝËN?ï÷=»Ä´?PÏÂÅ{?Q"‡ø&(É?PÏÂÅ{?ïúÛhús?3™ƒ'öìÁ?D'\ä\‹q?3™ƒ'öìÁ?ïýè›ï6?cA@Õ?0»((e<?cA@Õ?ïÿ+ÜI8û?Ÿr]7ò?"|er>
?Ÿr]7ò?ïÚ[•Ÿ[r?tŸö,{	?rÒ54qÏ	?tŸö,{	?ïýWð	›h?E9SêÚ§?5@€2¯Ú$?E9SêÚ§?ïü¶¿?-×IbßLü?<L"ÿǔ?-×IbßLüAGN4FGL J0237.6+0923?s>ŒoJÀF¨ÁTɅðÀ:XœóÀ<U¹}d¯­@Ij¸…˜@ù½ƒƒ­Ÿ?ÌÆôE·š6?ÆF‹?8Ð?üÙíçχ'@…Öf(¨ì¿£Mʟ\7u¿æ‡uÀ –ù¿á¡Ü>ñ§¿ãB–³5L¿èÁYAºµ¿ï÷yHÁ9òAGNbcuOD 58?ïøæUVk?PŠ¨VH%§?Lf©£dXC?PŠ¨VH%§?ïô¡k[Sõ?YN鱯Æõ?V½)·K•²?YN鱯Æõ?ïÙmQ'ò?s©"…+*?sIW¶÷K?s©"…+*?ïó>;ò?<¢mïè?Yƒûma;á?<¢mïè?ïóÔ5vÚR?V£x©(¿§?XW•YÃ;¼?V£x©(¿§?ïÓ1±º
?yõÄÆäð?vg';¹*¸?yõÄÆäð?ï‰E"–OZ?Œ3r^œaƒ?®·kš5~?Œ3r^œaƒ?ïÊ]L>ûq?dùŽâ¤H?zÑYÔӛ?dùŽâ¤HAGN4FGL J0237.7+0206?Ӊßc
§šÀI'•þÚfÀ;5‰+L"À<±&9O¬æ@µY5¦U@—?úÁҞ?ϵ8ªå?º=»aëW|?íUӌÚn?ÿ"Üj ¿ïÿMR™*?ïüˆFŠþÌ¿êó_s-F¿—Oé¢E¬¿å©Ÿ÷Ó¿ïÿú Âî'AGNrdgPKS 0235+017?ïý7õÔqÌ?R^2³ E?6@Q«›ÖT?R^2³ E?ïòÄ?#p?ZûÌÁ›Šš?[üww€?ZûÌÁ›Šš?ïݙJFp?l <ÚՏÆ?q3Zސt"?l <ÚՏÆ?ïïgL¢Š?E
ôñ{ãÏ?`˜í¨^¶H?E
ôñ{ãÏ?ïû9[¸¯×?D´.–ï£?CôU<?D´.–ï£?ï¼$Š¬t?‹còë0?€þ¶í#Î?‹còë0?ïÃD8ƒ?€ˆÑv²ëK?~ó\ƒæ‹?€ˆÑv²ëK?G˜å?|°QéÅ«?ˆXn++ÒÂ?|°QéÅ«AGN4FGL J0237.8+2848?ÎêYãÔ®ÌÀ<†E^®âÀ6âб§­À;<éõÒ@÷÷ÈÎæ@«9²©5?‹æ©¸ËŽ?¶NêÆÝÊ@(=îVŠPP@!%U¬ÿi¿Î¾üÀ'a¿àkÀ]RÁn¿åß:Wꢡ¿äp°×£Àd¿è6c¿Bµ¿í(/~ȲâAGNFSRQ3FGL J0237.9+28484C +28.07?ïõc/þ»?Qš±Ý‹?U9¢^÷H­?Qš±Ý‹?ï¾øÌ$þ?":ñä Šì?€A͍ƅ?":ñä Šì?ï³J5¿eÂ?ˆ‰-»¥6?ƒ-rG‡?ˆ‰-»¥6?ïøN';À?Rõ\/Ð+?NÅºÇ d–?Rõ\/Ð+?ïêt¡xÇM?bŒ;sÚ?e‹^×š°?bŒ;sÚ?îÍyÈp-?ºJŒb›Î?£(c{™a7?ºJŒb›Î?ïÍv¨eÃ?×E›pn?yD¬{*C?×E›pn?ïÇ÷—óô{?uæͦä?|4FT?uæͦäAGN4FGL J0238.1-3905¿ï¡m$_uÀP2ñVIÀ:B´½âN>À<Š7Âäì@Ój™üÀÛ?þÛ¬´('?º9@‡Y¦?ªŸbM–Ñ?ò'í"Ó8ø@!O0ï?ÛàÈâÝZd¿Þ"›Ãjxo¿áxkì¸$Ÿ¿ÙáN¹÷¿ånß{ûùá¿Ñ顙Ã5AGNbll3FGL J0238.3-39041RXS J023800.5-390505?ïÿ"§l7ƒ?EúóŸ³w?«N)‹‡?EúóŸ³w?ï÷˜«÷¦?Qï~…È}œ?PÏôü?Qï~…È}œ?ïùmK Ô{?Z'ŒöÅÝ?JJӐx¡ò?Z'ŒöÅÝ?ïþ	̘°¢?Á0Îá?/c7ñd<—?Á0Îá?ïþÚ³ë)"?ŽuëFv?"TÃÓë?ŽuëFv?ïÜWÓ6Ún?~"Š Ó?qÔIÅÕ8?~"Š Ó?ïûÁzðGa?R'æò''?@ú†ç'?R'æò''?ïûÓ{pAd?0Öë»Ð¨0?@²ƒ'ó‡?0Öë»Ð¨0AGN4FGL J0238.2+1531?îQ@h ÙÀD˜²é̸À:n­\ÄýÀ;ìg
ÑZ@)âøc!@n<c?Ê)^H4Í?Âá
6u?ø¢ê`[Šj@rK¡éõ'¿èe‰&"Ï¿Ýä8Ž¼ÆÅ¿ä
€¡{k¿ãUÌ»/¿í;	Uê`¿äËÀ}‰ÁAGNbcuCRATES J023819+153323?ïü ÜGØË?4¡_ûÒ7Ø?:ùR-?4¡_ûÒ7Ø?ïöjjR?VrCuî€?Sû+÷«ûÍ?VrCuî€?ïª÷3—uí?'§˜×p?…B3'àôÁ?'§˜×p?ïý•,«f?Ó%!nŒÈ?3VœW¸x2?Ó%!nŒÈ?ïùØÔB?HÒ²Éõ?Hœ®žÄ^?HÒ²Éõ?ïÔ²ôßf?€ÌJÐl—>?uô¦ˆOý<?€ÌJÐl—>?ïE'KF¥V?"Üâ·y?—M¶˜ã#A?"Üâ·y?ï÷P4‡x?Cµ-ÃO?Q_—b°?ù?Cµ-ÃOAGN4FGL J0238.4-3116¿ïÂr·¤êÀP•gÊêt~À9/f±%À;êmÀÍ»	@­ÙY"0,?ý0qLsv?§×Q
3µ¿kä#ü'?Ê]ÜT)@È/¨d7¸¿Ò¿º•'£Ü¿Ü.ò£¡¿Ü!HO$+¿Ú¤Š£ÝjT¿ßß­Ácã¿Å¡gÄ4w×AGNbll3FGL J0238.4-31171RXS J023832.6-311658?ïÿöª§ð?
qv¹€/½?%ñ‹…ö?
qv¹€/½?ï÷b*J4	?RÛ<Dˆ~í?Q;«¥Q]?RÛ<Dˆ~í?ï÷x'9?U©IÙˊn?Q÷zI,Ò?U©IÙˊn?ïÿ&IH{ø?ÎY­ !¢?6ÞךêÕ?ÎY­ !¢?ïþWizå?X¿
ÿ°à?*‰lÓxo¡?X¿
ÿ°à?ïÚ£@¦'5?vs	X_Í?r®_Í8¹?vs	X_Í?ïùî"
CÙ?Sk¾?öx?HEð &†p?Sk¾?öx?ïþñ?Géy?JüMù(? ìFÇ|ð?JüMù(AGN4FGL J0238.6+1637?¬¾\ÀC}'Ó"À7¤l[ríÀ:þm'JÈ@(ôï֒@·{|x £?f÷'`¹v?·‰.'dœ@(æOTÑé@!#…k9_¿Àòèn¿Ý;'¢‡(ÿ¿ã7GpxŽ¿âVûŸs"a¿çñ=Å]m¿çÇFê AGNBLL3FGL J0238.6+1636PKS 0235+164?ïòW €Ü'?Wži'3×o?[Q¿|¸{r?Wži'3×o?ïÆ0•Áj:?™Y¬B{?|çµ4˜v¤?™Y¬B{?ïKs–z«B?•2h&ß?–'2beÁ?•2h&ß?ïù%gºñ¥?T"jšÉáˆ?KjbPÜ2?T"jšÉáˆ?ïé°°ŒzL?a›š*±*?fOO¸=ãT?a›š*±*?ïCGG3½"?§"ßêº2?——±'?§"ßêº2?辶{¦ø?‹t§Égz~?…–aIÔ±ß?‹t§Égz~?ïË=#)®X?v´p:³?zan‰ecñ?v´p:³AGN4FGL J0238.7+2555?í_#=>FÀ>üú½ ßßÀ;ÙÛ©¢À<…'e²@!!þ}sô?ÿ¤óÕORN?»äY€¿¤•Às"?ãI›árv@üó€À¯³?ïþvÞ-È:¿ëÃ<?ÌHÿä>>I竿䊗hfñ§¿ÏYm3࿦K_
7ÎAGNbll3FGL J0239.0+2555NVSS J023853+255407?ïþ(Õ¿Ã-?!½L͌¡c?-r¥IAÎL?!½L͌¡c?ïõT
¬ç?UHÓKÒ¥?UWÅ|2ê?UHÓKÒ¥?ïî/ÛºÑM?_æ#ûÿµ˜?aÐ$§Òó?_æ#ûÿµ˜?ïùdìy÷y?3b|˜kbB?JlNU´µ4?3b|˜kbB?ïþ=«S?$¤ZSÖ(Ë?,%Mô'ˆÍ?$¤ZSÖ(Ë?ïÑhƒÞ,­?x×ÒPÔ?wK¾Ëa´?x×ÒPÔ?ïñIûso?e]-Ò©	>?]l¢ [?e]-Ò©	>?ïÔFúÌu ?kmíèª?u܂‰G?kmíèªAGN4FGL J0239.5+1326¿áFòÄÇßlÀDØ΢âaÀ:ú–xHÀ<là‡"´@û-8¦?ÿâZµX<?Ñ´`YÜë(?Ç#–=áã?óV]Ú¦ª@žÃmþ`C?íñ'QS…¿în16ñL?Æ2ØÅS†»¿áô²YƒÿÔ¿ïÿæ¦Sf?ïþùÛ"ÐåAGNbcu3FGL J0239.4+1326GB6 J0239+1327?ïõñ¶ça?_N̛îkU?T'¥d'?_N̛îkU?ïõÐ玚?W²
¹ÍWÀ?T^1ŧS?W²
¹ÍWÀ?ïu
f×
Ï?Š2ƒ^9‰H?'^S+ýÞ?Š2ƒ^9‰H?ïþzYëâD?q8wؕì?(Z_‡ÚÉ$?q8wؕì?ïü¨øå¸	?@T÷‡ùúX?:¸7§/A?@T÷‡ùúX?ïڞ ÙBÁ?siEF$¢?r°¯–O¢?siEF$¢?ïHZ-.G¢?"{;pՑ?–ôº_^u±?"{;pՑ?ïüý·CÆ?/

Ò{°?8S"»W?/

Ò{°AGN4FGL J0239.5-1353¿áúK±6÷ÁÀNÃ3ÁÎl	À;sýþžÀ<we'+@¦œ%.@œløPß?Ƭڝwö¿« 8Bf­?ã#û½{ 2@Ý»´MпÓ
e@¡†¿ë䩘^\¿æÏ€Ü3r¿âf="†¿ïL_ŸLáÛ¿îµ{aöDAGNbcuCRATES J023939.13-135409.6?ïüÌ<ë)?55fd·?9ž–ó^ ?55fd·?ïïÑÇ]w*?uÁµ"î$(?`.8yM†·?uÁµ"î$(?ïÕT$'Ò?xÊô=¨¤É?uUí×cE¡?xÊô=¨¤É?ïû;Áæق?0 ŠžŽ± ?CøÄBJ?0 ŠžŽ± ?ïý"ƒ?<,®ÞËÁ?7ڃE3;?<,®ÞËÁ?ïÇÜQò]w?ˆS£…±}?|×p,7?ˆS£…±}?ïÛ83^br?}ÃFó?rcæDp/?}ÃFó?ïÔF–_?i}ÛCÑDº?uÜõŽâÜY?i}ÛCÑDºAGN4FGL J0239.7+0415¿íҚðfÛÀH'øã¬cÀ9ƒÇhß½jÀ<4Dé>›@~UñN6@ô±$Йá?±Š*!!ôÙ?°ÃʀÓ`K?ö‡‰	ÿ]@_Ÿ —$I¿ÄE¤¤å}¿èTKç_J¿éó¦öyn¿æûÖƒó?¿ïþ©žttÇ¿ïßÂð|AGNfsrqPKS 0237+040?ïþ4|š–€?!å^ž¨^?,¸9žžâÚ?!å^ž¨^?ï÷…¼±»h?QÇa9<ø?Pô†4?QÇa9<ø?ïãÙDï,?iâJ‹ª;?l&»/0d5?iâJ‹ª;?ïÿ:ݘïG?àFqi"?¤T3qå?àFqi"?ïÿ†?b¨ÛW "?Ý9ÒbôÉ?b¨ÛW "?ï×UÙa—?wb#liQ?tvT÷"hº?wb#liQ?ïæ°T,cG?qjEË<?iO«ø¸E?qjEË<?ïþòàv'?&%z½eá?.àÑæÿLÆ?&%z½eáAGN4FGL J0240.8-3401¿í¤'I'LÀPcˆ†aÀ:øg³À<À–Î
>­@ó"¡ëx@œˆFŠþÌ?¿'t Õ'Ü¿¬lB|?îMâÔv?þ/r†r¿â0'9¿äC#k?;¿åsþwY¿âö?ç̂¿ÜtßzúG.¿Ü䜢7£AGNbcuNVSS J024047-340018?ïýžËK‡,?#V¤ô=Ì>?3	¦õSs"?#V¤ô=Ì>?ïóh.´ë§?ZwøOSš?Y/¢·$ñÞ?ZwøOSš?ïíÞUòa?Rðà1s?b!ª^˜Ï?Rðà1s?ïú^íûq?0Ïov¹?F‡ëոר?0Ïov¹?ï÷©TÄö?IpaŸ˜'Â?Pz­Vv•?IpaŸ˜'Â?ï¼X
ƒ?'÷Bõ¦"[?~¡Óí³?'÷Bõ¦"[?ïë«Í×Ax?jš§'°µ?dT2ÂGµ?jš§'°µ?ïÉ@˜Ìj&?p—"Q`H?{_³…Ý0é?p—"Q`HAGN4FGL J0241.0-0505¿Ã3k–•ÇíÀKìØ]ú‡À:±²dkºcÀ<'£¤µW@µ×‡eåb@]OG"=?ÅAæ0 .?Á±Ï…ä°ï?ú\œÓà½E?ÿÈaMw×þ¿ï˜?ǖ,'?îóÕðaýK¿Ýá,Ö!à%¿â2ƒ
¿ä:"DÇ¿ânA§VAGNbllPKS 0238-052?îLd;V?ÌqF°?«?‰¾ìJ¨?ÌqF°?ïè.ùnk?k}ÏJ=ÙZ?gÑù3ìlS?k}ÏJ=ÙZ?ïÏW¾ØÃP?€«Ii´À?xT |ðì?€«Ii´À?ïƊnê¡?a'út•ö?|ºÈ'ŸgH?a'út•ö?ïá+'?u¬¿
tQ¦?nÔôã&7?u¬¿
tQ¦?ï¢G°IA?Hcu‰ÿ?‡n
[»Æ?Hcu‰ÿ?ï¡®ë)H?ŒAYñËÐG?‡"E2>_š?ŒAYñËÐG?î·³Îª?"=ÎÆ
á'?¤"Î*vÊW?"=ÎÆ
á'AGN4FGL J0241.3+6543¿Ø"Hsü@éh=;À93?Æ¿l'À;˯bXº¬@ 	G…z¨¾@°Ê1u?°‹lÛ Ú?£^î^(:˜?ót‰Y°u~@áj5¨ÙS?ìtxwàâ¿Î´
^'ӄ¿á`¢' *¿á'æ™ýl¨¿á׆߭¥¿â9LÝ~JßAGNbll3FGL J0241.3+6542TXS 0237+655?ïüt~E‰?/Z¶)ŸeI?<[}á–Ù?/Z¶)ŸeI?ïåÚú¯U?o_k̵z?j%9M*?o_k̵z?ïó³ŒÆÈ?O"p†Au?X˜æ&ù0³?O"p†Au?ï¹^ö,S?ls¸4̧?¨yÇôKC?ls¸4̧?ïñÓö˜^?TWÛ§dÂ$?\YÕޕ3p?TWÛ§dÂ$?ïR
~´?¡2G±†?•¾°+5˯?¡2G±†?ïãªT&óµ?w5."ñÏ?lU«¶°3m?w5."ñÏ?ï]h]Xî?‰
§Í'ÕK?œtRðåFE?‰
§Í'ÕKAGN4FGL J0241.9-1603?ìh\IÏNTÀOýüÁrÀ:Õ¦Zr<À<'æ$Œ§C@ Æ*uIƒ,?ù²¶»éOº?ÑmÝÞÂî}?Ãñ¢õŽ?ú4°%Í#@(·'㟢¿ïþ"ÖúÎ?ïÿ×hE¿çånÿ½¿¦qì™­ç¿Öý€^_0è¿ê³Ù¡FŒ+AGNbcu1RXS J024151.6-160339?ïÂ	À;û?±Ðx"Ò"¿?~ûçÃŒ?±Ðx"Ò"¿?ïó'Õå'Ú?[ÆÙ-"MÒ?Y°T°¬;Ð?[ÆÙ-"MÒ?ïÙ#§úÛS?{•¥4'²ö?sn+ë4þ¥?{•¥4'²ö?ïõtƒ,M??Ü[T?¤?Uùšõp??Ü[T?¤?ïý®ŒDòM?/2"ÚÿÖÑ?2‹œs6É?/2"ÚÿÖÑ?ïïÓÓãS?‡Yiþ¡[/?~(ÀÂÅ?‡Yiþ¡[/?ïЈQ*%?{,4/jMg?w»À;>!}?{,4/jMg?ïÔoAðÿ÷?k"¶¶ò?uÈ^÷±Ð¼?k"¶¶òAGN4FGL J0242.3+1102?†ï[Ð'¤ÀE¥ÄڐïÀ9¾½¨!óÀ<1Š¼‡@X:þُS@{ÇÜ£¦?ºýT)"
F?Ï+WÝ´>@Έ°=@$'w=N?¿Óh'cëý¿â¤ðñ5¿æ¾ð֗Pê¿êðþÊô¿ïù•¸c‰<?Ú6†¤ÊAGNfsrq3FGL J0242.3+1059OD 166?ïØWnj°'?›¤ ,܇?sÔH¾ù,?›¤ ,܇?ïóŒ¨"?bÌÀyã‰è?YùÚá0[»?bÌÀyã‰è?ï=C0Æ
U?Žf'"ÜÑ°?˜W™ìfc?Žf'"ÜÑ°?ïú¦.¨_?2&oáƒ?EgFUç͋?2&oáƒ?ïⳝ&?i3> š?mLb¯!Á?i3> š?ïÑZ!xd"?[=}ö?wRïNÌ}²?[=}ö?óºf?Ÿ¨Ôô.R³?¯Å6X™?Ÿ¨Ôô.R³?ï×ܔ"Ë›?dÜÑ%nÈä?tµMÞ¦?dÜÑ%nÈäAGN4FGL J0242.3+5216?É;XŸîPÀÚñˉ֮À9mmþ
\zÀ;²'쮤@3éހ~@_°&£Ø¸?¾ÁCכ1õ?˨]ס'@VùzªÁ@²¨ÑÅÛ?ïÿn	È֞¿ß"]ó%Q¿éßø…–W¿è,ñÀw)¿íA"d~.Ú¿ïóãðµAGNbcuTXS 0239+520?ïÒâÎÊ[Œ?p•ÎŒ¬''?vŽ˜Óz?p•ÎŒ¬''?ïꢃ«¤<?lřqŒ$?e]|8Þäj?lřqŒ$?ïSºÆK9 ?‡
¬X?•ˆ§3)/÷?‡
¬X?ïÒlŒ¬\?Z"‡ëošÛ?výIÊ'ñ¬?Z"‡ëošÛ?ï¼ÎàM]+?')ñrHôÈ?€ÌGò€8?')ñrHôÈ?ï˜bøGÏÍ?'ýP[Ñ?‰çAñ{¨¤?'ýP[Ñ?얺Ò܏?¤a_F…¢ ?»J/	i‰?¤a_F…¢ ?îÃrɇY?‹4"À+?£ÎˆÔCqk?‹4"À+AGN4FGL J0242.6+1735?ï蕉OۜÀBã4›èÿ2À:8.©`¶úÀ<-V@½XÛ@y÷šÖ°{?ÐÿR©úe?Ö‰bÙ?þåä`gHä@;ݹ"¬?ʲî)hÚ	¿Ö¸Éà‰B4¿á^'ျ¿åQ)=f¿íî6ߐð¿ß¡¸¡òƒ–AGNbcuNVSS J024248+173700?ïê¬å·ær?_ç]"×"F?eSL9?_ç]"×"F?ïô·¬ü?Y;70^º?V'ÉüŒ±?Y;70^º?î0Ì:› ?™Ç"y…W6?¬ó<^fMù?™Ç"y…W6?ïëKÊÑ€?IþÁˆ¹H?d´4÷ïÀa?IþÁˆ¹H?ïîcýÍÃ?\~ø-£§:?aœ0Ý­?\~ø-£§:?ïÔÛ|=Z?yu)Á?u'A×'þþ?yu)Á?í+ý¨ü|Ø?¥&Šu'½Ø?¶ ¶Ò>Æ?¥&Šu'½Ø?ï±JA[ƒÎ?l䄑"(B?ƒ­o±^n?l䄑"(BAGN4FGL J0242.9+0045¿Ã¡cꂌ¯ÀI¨	ÃÎ ŠÀ;;éÿãzŽÀ<¤§:l™@±)Î/£?ÿÚ¹šû?ҏ¡·uM?ÃjÔL?ô˜çÂòXx?úiè‹Ï×?Í$Cy|n?Í0"W=(ª¿â~Ȃ=¥¿Ì­W|Ë	¿ïÿwy´!?ïõgÉÉãAGNbllFIRST J024302.9+004627?ïða9Uâ
?[ho?ÔÝb?_=gy¼P?[ho?ÔÝb?ïßDé¾ö?z´UòϺ™?pp]¦dà?z´UòϺ™?ïÐães*?""1$Օ?‹Ç0ò	t?""1$Օ?ïÂç;ۊ?fm†Cc™?~Œ@žß?fm†Cc™?ïâ½aAZá?mqɆEMÃ?mBžá78?mqɆEMÃ?ï~¨B?©ÚLÝÁK@?œ?a©?©ÚLÝÁK@?ïw0ñí÷?Ä?Á~=‡?'áÂAo?Ä?Á~=‡?îL};êçÀ?œ4ÏtÚ¸í?«8,B-k?œ4ÏtÚ¸íAGN4FGL J0243.2-0550¿ïÛ¯¥ÀKø§Å¬GÀ:Y¹'†¥¡À<aß 'á@|7ýÈBO@Æ<ÓG?½nÊc?"KtÈ~ßY?Ñ÷œ§@ @1|ª¤¿°àøûÔÍ¿éÔ¾³¯o¿êx/â縿é§ã¿³	¿ïÿúVrÓ\?ïÿânÁŒAGNfsrqPKS 0240-060?ïû	Vüø?qÇ
wb9=?CÚ¢þ1hå?qÇ
wb9=?ï÷ '"7?U.e§ÒQÿ?Q¾Úr/"ÿ?U.e§ÒQÿ?ïÙ
ü;?woAóg°±?szå>¦ã?woAóg°±?ïÿ¦"\v>ø…
\$(?Zñ°Ð}>ø…
\$(?ïþ~Ô­}
?,ÑzpQ¡~?(´[¬ßm?,ÑzpQ¡~?ïÓb®\0?ya9XÇ.?vtNµàl%?ya9XÇ.?ïá{¾ù`»?vÍ
«›Í?n"@ÈÆMš?vÍ
«›Í?ïþO]­§?$/0Ò3Ç?+
&ÒV>p?$/0Ò3ÇAGN4FGL J0243.4+7119?ï7üµC@$Ȓ‰ÚßµÀ9¡¬JvE×À;àf$ø
@Åo!JþV@-[h¢×?´˜Áò#?ª_z@ò'Ð(¡à@›ÅB궿ïýQœI?ïþI|JÔ:¿à­‹ßÙпßÖ³jû÷]¿æ"…€‡ú¶¿ämNí£ÜéAGNbll3FGL J0243.5+7119S5 0238+711?ïý
Â=Ë?3«ô`YU?7©ïí'Á}?3«ô`YU?ï척Ź?nŠ—pd	?cêMJ½fÉ?nŠ—pd	?ïØv+¶?sÖ";â)æ?s÷Åu$Ö?sÖ";â)æ?ïø÷0+I?5ÕÕ@n‹?L#>—bNv?5ÕÕ@n‹?ïú@wO˜?D¹©Þ¿cª?Fÿ—2â¯{?D¹©Þ¿cª?ï†ÛÒàHf?œçùS?ŽIK]'"?œçùS?ï}ÿ€qf?Q3ñѱ?@±©¡H?Q3ñѱ?ï堅h–?`¯R÷r_'?j_z–'ó?`¯R÷r_'AGN4FGL J0243.7+0321?çø"y']ØÀHœ¡ô±îÀ;V¨°ÑåÀ<¬…\ '@H.ï><@šMô™?ÔçB.x¹O?Ófæ~y­–?üõO؅g³?ù¸0—!š¿ïÕv‰Ê½?ïÿEZ}$¿âîGÜ7£Û¿Ø8OfÆ¿ïÔF"
q¿î·N: AGNbcuPKS 0241+031?ïÛ\þ;b_?koSl[?rQ€ó|ÜA?koSl[?ïg'ò7jz?z["ÃÆ)?"¿ñè¨?z["ÃÆ)?'$²?"©ÃÐ}E ?¥G÷ÜãÜ?"©ÃÐ}E ?îÞØÚïqµ?ƒ{ö|èì?¢rRÀ²±?ƒ{ö|èì?ﮍû'íd?€™Éêk*ˆ?"\&Û\ð?€™Éêk*ˆ?ìïkb¤í?Á´þ"?¸"¤é#²œ?Á´þ"?î7Ê­Éã?žþè!ԁ?¯LƒYnäÃ?žþè!ԁ?èu…ˆô
Œ?¸žàkRBõ?Î)éÜ/ÉÐ?¸žàkRBõAGN4FGL J0244.6-5819¿ÙàšC&ŠÀJ‹ …±…À9º'‰)ßÍÀ<0?\6a¼@ ‹'6û"¶?ûÜ ý¦‰?±
Þoú?¦å|."£?ø‡¿|'2@
€†µ‡Œ?ïaL'HD¿á§©Ý^•b¿Ö#ø'Äj¿ÖH:	ç
¿áÈ4ˆ¿ª'_ÁåÕAGNbll3FGL J0244.8-5818RBS 0351?ïÿTô׋?
*˜´á?µfdãpÍ?
*˜´á?ï÷œk}sì?Qql Žj?PÇ)3Òؼ?Qql Žj?ï÷ €Ç`?\ÛÖ±[?P¾þ8ÏW?\ÛÖ±[?ïýçÁ¸$?½ÅÃ;•z?0Áø¥Šƒ`?½ÅÃ;•z?ïþÅ¿BÝ?ùñ¹{?#¯¤~+šÍ?ùñ¹{?ïß»ô¯·5?qÔÿºJ•+?p"ˆ‡ýÖ?qÔÿºJ•+?ïöšZׇ?eÓ.;ØÃX?RËJ_­a8?eÓ.;ØÃX?ïüÓ¼ÄÛ«?,fLãüõÐ?9bGEÎó?,fLãüõÐAGN4FGL J0244.7+1316¿ë6ϟåäÀDÍ_™Ã‹À:h¢À‰ÈkÀ<+ò£ +@¢|f-@Œ°Úþ¾·?ÔR°+¬V?ÐVMênžC?þ¼g#û‡Ë@
Wxelì¿â^lg1g¿ã5V=ú6'¿åɓAÄ¿ç?¡k2Ë¿ïÿyݼ‰3¿ïûfKŽtAGNbcuGB6 J0244+1320?ïøa&Ð=4?Eòw°
%?N{e§
jT?Eòw°
%?ïô'KûÓ?[Tý¹ÐÚò?VÛho¢É?[Tý¹ÐÚò?ïÍoïs8?gÄÍ* ª?yHeÕËè?gÄÍ* ª?ïñµ)ß?B‡éÂîÌ"?\•ýÅBb?B‡éÂîÌ"?ïûÆp£g_?;×i6d?@æ=öà@U?;×i6d?ïÔp€×¼ü?w΂>å?uÇ¿¤Ÿ¡æ?w΂>å?ïGu²´¬?'`Z¶ÛÍ?—I¥ü®†?'`Z¶ÛÍ?ï³Ôô—É?qé6ÏÇÁ?ƒ
ÂÖp»Ý?qé6ÏÇÁAGN4FGL J0245.1-0257?î¨Ú&§‰œÀJÏohیÀ:B˝!äÀ<oNÇ
p+@ޙÙ/†«?ÿ¨×úþ8?¿uÁ"I«ñ?¾8œ(À@ý"$½@
ý
ÒÁÙ¿¸ª½¬s?ï]&š¯™¿Ó86¨¿âѤÆôF¿á4C~"ë7¿à¯3ß«v¼AGNbllPMN J0245-0255?ïþêp™¬?fj³Œ?!Xõ³ú"?fj³Œ?ïõMØX¤º?XŒ3!dž?UdOÍ(*?XŒ3!dž?ïôÃæ
)x?Qʉ?Vx3«ó 6?Qʉ?ïûšáJæ·?(ÚµÇ(h?A"{D+3?(ÚµÇ(h?ïý=¿—ôÃ?3[Ågç´Â?6y†Ä?3[Ågç´Â?ïÔ®c'?ƒM@¡?uó(Ú&k?ƒM@¡?ïï6ð	Æ[?lO¶A0ÿ?`É	wtï?lO¶A0ÿ?ïöDÃÄ?DK›"=·P?SçuûpØg?DK›"=·PAGN4FGL J0245.4-5950¿ìÅçÁÖà³ÀI÷\¿ôw6À;#£Ï}5À<ÏÓ¦Û¡|@,¸aúœ?ýQ3~²†?Ò7'ßm
u?Ó¬ œîã@1õ`iÍ#@ñ_	zÓ¿éÆk>'aí?îþQ>¶ôô¿×3ŠÜgtƒ¿Ø§¢Æ¾ì¿ê¨^=¢ø¾¿ïò'šx¼ªAGNbcuPMN J0244-5948?ïï#VqPÐ?ZY¤ãWn?`Ü©PÖ8/?ZY¤ãWn?ïï
Ò%§/?_¤m&~d?`ò-ÏZ?_¤m&~d?ï"D•'¼T?¨ö|ž4'?ŽîÚÃÏZî?¨ö|ž4'?ïˍ"b./?`p¶šàd?z96O˜Ô®?`p¶šàd?ïÒ{ mïÙ?oÆι""U?vÂoن3€?oÆι""U?ï½|"÷b?ŠQ.Z6é?€ ÷>_ì
?ŠQ.Z6é?î©·˜O?™_é–ÿWÜ?¥dŽ2Ü?™_é–ÿWÜ?ï6Œ!>œ¦?‰üL¾µâï?™.{ÑM3;?‰üL¾µâïAGN4FGL J0245.4+2408¿ïmeÃ07À?ÐaAcwŸÀ9«Ut¦›
À<ÁJ¸Šö@>ÎË)´"@._#|?µtîêXùÁ?´ý"€¢6?ø'"d¦rÆ@¸øU'¬æ?ãºO¼Öµ"¿äk^R›®G¿ë¹ÒߋkY¿á²¡bÃÝ¿è"£Y5ü¿ïöŠþøïAGNfsrq3FGL J0245.4+2410B2 0242+23?ïþÀ9bï†?SKÂ!S\?#üië0w?SKÂ!S\?ïöæ糶"?Sžé"Å­¾?R20íÉG¸?Sžé"Å­¾?ïÝ­oºM?tÚêÀ%f?q)HÊïá?tÚêÀ%f?ïþÊ(Ѽ?Te0ȹ?#]}Åî‹?Te0ȹ?ïÿ
ð6<?ÀVN¹²?AñÕVqn?ÀVN¹²?ïÔê­TÙÃ?OË<ziß?uŠ©tš?OË<ziß?ï¥îŠäh?…Rrή†?†"]_fê?…Rrή†?ïüjà&N|?0dS­àã?<©µ‹¸?0dS­àãAGN4FGL J0245.5-4502?Üò6±,DÀN‡|í'hsÀ:Ð$qÏP5À<sóëõ‡@æ•â@÷ퟫ+'?ÄX½L&I¿°Ôí=ì°Ô?àíX]'@Z¹D.Ù¿ÂÁM½£7¿è>}i7Q¿êþdŸg¿ît¯45'²¿§".ÜÈ~›¿Ô CVìÌAGNfsrqPKS 0244-452?ï4`ˆ'‡?¿¹µó_?™sîæÝW$?¿¹µó_?ïõ?€¯¤?eÂfüÀ-Î?U€þ«¶¹z?eÂfüÀ-Î?ï˜0²¡?Š^­ö¢ýÿ?‰óøš6ö­?Š^­ö¢ýÿ?ïÿYô+û?§¢oª?Á}b)~)?§¢oª?ïûbr©Î?T<!²lû?Bv6žB—§?T<!²lû?ïÇzÓZÛn?‰ˆ/M ?|B–b`}?‰ˆ/M ?°åvÎ?Š3ÿkB‰¶?‹ÞÓ¸ãܕ?Š3ÿkB‰¶?ïó3õŒå?U
º__%?Y˜U¿´'?U
º__%AGN4FGL J0245.9-4650¿ßå–êŠÀNàC¢@À81Êx^¶oÀ;¿Œæ,ð#@­{MÔ@w¹Z)AB?¡™ÿÅój?½Vö†Úz4@%4z[ñ@0|o'4¿Ðnb×Vi¿ám=¾§p¿æL"üÅ¿ç}Ëb>Ž†¿éÖt€Û\³¿ìûgPAGNfsrq3FGL J0245.9-4651PKS 0244-470?ïòlFOD·?z!Ìæg›?['sd6B€?z!Ìæg›?ïó;;óÔ¬?c>GôÃYY?Y‰ˆŸW?c>GôÃYY?ïØ·¬$x?u5A\ª?s¤)ÙÚß°?u5A\ª?ïþèãÙ®³?¹b9ÒVõ?!qÆOÖl?¹b9ÒVõ?ï𬷝T~?V°(­ré?^¦'L³Z?V°(­ré?ïÕûלñ?yPWGmßx?upÃ+Ã?yPWGmßx?ïÕö®6x|?~'Q*ýË?u©Peì?~'Q*ýË?ïûE°…»¹?:S¦ªd®Ä?Bé=7~è?:S¦ªd®ÄAGN4FGL J0246.6-3348¿ëþ‰¼héÀP–=Ć­À;Òh;R¼À=ØL\Ïå@!«5MiÀ?ó÷ ›šœ?é£,àˆÁZ?֍˺Óûë?ë½Pù׳@¿¼§»›L?ìoè%ç}¿åú9¢8#³¿î†9[e?àçŒ Š9)¿Ö‹ 1¹6¿ãÒe}ˆAAGNbcuTXS 0244-340?ïú2õ[óW?@§|Ú4¸?G4*þ&#:?@§|Ú4¸?ï÷M\́?QQÉXÉyÂ?Páeže?QQÉXÉyÂ?ï¼'é¸Q?°ÛIN<ù?€ùNØݪ?°ÛIN<ù?ïþsX<W?kß/¾?(Ê}"h™—?kß/¾?ïûE¸"QM?CQxKÄx?Bé9ø6I?CQxKÄx?ïÓD·PJ?=yl"?vvݱf^î?=yl"?ïÆʅ'zK?€€²œ¼»?|š½…
_?€€²œ¼»?ïû"Щr¢?AR"6-	?A¬½]äÇ?AR"6-	AGN4FGL J0248.0+2232¿ÇŽW_ý'À@r9¼º0À:ތ]pô_À<]ÏX˜GŠ@ }¼Î§îF@1jWX?ÈS¤|Ü?£ËF¡
bk?á(2F@̲-9I"¿äDÌMKn¿â՝ÖÀ¿äj‹Û¿à²Ál!'¿Éµû$#ë¿çÓû?PøÁAGNbcu1RXS J024800.1+223136?ïþ1ââI?*á/~…?,áÐa2Ú¸?*á/~…?ïôÅ-Šìq?WÙÌŽ(?Vu¥$œþ?WÙÌŽ(?ïõ¼ \R?Cԝc¼Tà?T†¾Q\H?Cԝc¼Tà?ïû4£9šD?,´ņV:?C-r4WfX?,´ņV:?ïþ[:°¢?#¤›îòR?/zMp¢d?#¤›îòR?ïÒ‹ÔN?ƒŒ1mµ‹û?vÀ|XRhä?ƒŒ1mµ‹û?ï÷u4?^½ÛRُ&?QË^¬HÌ?^½ÛRُ&?ïà™hÕ?bõ‰]M[?ofã]¸ºî?bõ‰]M[AGN4FGL J0248.6+5131¿êñ>ÏðÀçX}o—hÀ9NÎþÖ4UÀ;ÎDŽŽoš@N°A¦¾p?üçC:è3[?³YP¢"Ð?ÀÌê(þ&@©NBƒ2O@OZTŠEê¿á©åan/¿ãQzç&ë&¿ßÇRÅ؈¿ÖÔµÏZEÇ¿à=ÁA(iV¿éÊKéžtAGNbcu3FGL J0248.4+5130WN B0245.0+5118?ïðlö3´Ÿ?`)ÈO?_&¦U2Å?`)ÈO?ïÇP‰M`?€eû€–Ê?|Wô[¥£Ù?€eû€–Ê?ï¼dÒ½|£?€âqjù"?€æË\ÿo??€âqjù"?ï›ùñ9?l‡i#+¿|?€Ã"&Ú?l‡i#+¿|?ï¨á?öe"?…*nûÿ¹?…Ç°"Â?…*nûÿ¹?îƒ
?±GW¯‹Àµ?§È\k=?±GW¯‹Àµ?îè0`Έ?š
…qûw?¡|ùò< ?š
…qûw?ì»ÆõÎ? ¨ƒnkÞ?º!ÏQr? ¨ƒnkÞAGN4FGL J0250.2-8224¿ïû;>^NYÀ@Ӗ¿Ê…ËÀ9Ô	:;e1À<K›•ó@ŒGœÌ©ç@ÜÈÞ*Ã"?·'Ž zÚù?¯Åìûw?ó«TA ´@@ŸÇ™‡%#¿ÖÌ`it¿æõ®j}¿æIRŸ48A¿êA<ÀûˆL¿ëM'Ÿ'ç¿ïîxžwNìAGNbcu3FGL J0244.4-8224PMN J0251-8226?ïþ«d¥Ï?yÔn¨]?%I¸J†,?yÔn¨]?ï÷>7?©±?U‡«›|Û?Qƒ'Õâîu?U‡«›|Û?ïÛ$°R\ˆ?yLµ1oú'?rm§ÀÔ<?yLµ1oú'?ïÿ\Á÷ܛ?ô>à+®?gÃì'äã?ô>à+®?ïÿÜ–Ç?HÆ$jÌ?$b'îé%?HÆ$jÌ?ïܾJº±?}Ôßç˜íX?q Úž!3Æ?}Ôßç˜íX?ïíi@5?hÜËi•°Ú?b–æß2p?hÜËi•°Ú?ïþ'û>¼?$ZÒ¥=zò?-€H¬š?$ZÒ¥=zòAGN4FGL J0250.6+1712¿æ¾cݗl»ÀB‰‹`ñ²_À:àϹWÀ<*v­ÜF½@ ´¹‹Q'T?üB # –x?¼H%)Û?®Ÿ
át=ƒ?òÈ¥‹?cÃ@Ë:¦o¿ÓÏ"'|¿å¨HÞì	(¿Þ'1£X¿Ô¯$f‰¿á™Ÿ]þ¸Ø¿ÓyA쉁AGNbll3FGL J0250.6+1713RGB J0250+172?ïÿ±¢?
"ïæëH?Iåˆ;+ø?
"ïæëH?ïö-ö!H¿?VT&ncëÏ?S¤6½Ó?VT&ncëÏ?ïùã¹ÖÙt?L4ëg`eT?HqÖ¡MÔ?L4ëg`eT?ïûí¶ž¯z?'Rÿð¨V›?@I$àá"Í?'Rÿð¨V›?ïþ'¦7Í?!¤
É^?&åŸnð'ÿ?!¤
É^?ïÚÎÊ D%?sþaòDÊÅ?r˜šñq ?sþaòDÊÅ?ïûú^%È?Jp]QCæ#?@òÚøû	?Jp]QCæ#?ïôúl±óÇ?ES¹ÚA]U?V&ÐR?ES¹ÚA]UAGN4FGL J0250.6+8435?ïŠßŽ_BŸ@6ir%·I®À:	L‰EŽ€À<~ÿÕ7ÕY@zR½'¾?ÿ¾Ø»gJ?½{ ¡yüŠ?¹íߨ,ì?ý<<& ûù@ð"W_´?Ë©©\/UÙ¿áe'¢xæ¿ã¨üþÿ޿כ#¿äÆ÷ µî¿ïÿ
!ANAGNbcu3FGL J0249.1+8438WN B0239.6+8423?ïý¹/ÐÁé?"™†T'†Y?26 
i?"™†T'†Y?ïñ¦² •{?Z´²TžŽ[?\²š[àJ^?Z´²TžŽ[?ïõˆz.ç–?`	i®?ÿ?TïxõƒQ?`	i®?ÿ?ïٝ!.?Uˆ0V½k?s~1C?Uˆ0V½k?ïü'˜Û?1ŒN'»?;ïÕhÄÌ?1ŒN'»?ïÄú‰Û?'ÍëÓ?}ó'Ûz ?'ÍëÓ?ïïZ­íÛÞ?sW)×Îã?`¥QïÈ
¬?sW)×Îã?2Ô?s"Ä­Ïr£?
üªÑs|?s"Ä­Ïr£AGN4FGL J0250.7+5630?ém<«å"ÀíÊ"Îa"À9ÙÓr²À;çÙÉ4'Ø@ ˜ù(öCi@Büý@´?¾2ÿܙžw?¡]¡à~Ê$?á/¯4_?ôlÃk$;¿çë«_>ÔÒ¿Ûï—<M¿ã'#? )¿Ö2£uæa¿â{ÒÿkÛp¿ä	•ª÷ïAGNbcu3FGL J0250.6+5630RX J0250.7+5629?ïøéߓ_)?BA•¹?LX' vÛ
?BA•¹?ïÇ
íBQù?"{ÈÀ|)?|y	c¦w‰?"{ÈÀ|)?ï×öòQ'?p³þmܗ?t†öG{/?p³þmܗ?ï@䶚ӣ?€!Š±Ð[?—ãi*í½©?€!Š±Ð[?ïðS/…‡G?TŸ¾ÓŽ'¹?_Y¡í²µ?TŸ¾ÓŽ'¹?î"þ"!Y¹?²·":ëõ?¦°¹žáq?²·":ëõ?ï¾ÏåIŠ?"GO]ôÂ?€L;ŒÕm?"GO]ôÂ?ë{é€üâ?©=*5"2?Â[™üx?©=*5"2AGN4FGL J0251.5-5958¿î½ÆaΧÀI¥£3vOÀ:ËGxd•¬À<»É{´Ú@øTD«@ÁÅàIS?Ç)%=QD@?ÃzO|jÝ?ùͼì"øù@

yæ ¿çOÊB®Ñ9¿åm÷T_Ó¥¿Þz&ÂaŽæ¿á°.fDØw¿æŽ"¬Ï¿ïÿ¤?åÉAGNfsrq3FGL J0251.5-5959PKS 0250-602?ïþl
Pw"?$ÐÙK1=ý?)?Yùw­Å?$ÐÙK1=ý?ï÷ç¨ÎÉZ?Q!ôD&ŸÎ?P0®䁙?Q!ôD&ŸÎ?ïì•e¾†õ?kÚý!м?cjš#<{?kÚý!м?ïþÑãÚR?*…Õv¡?/ÒßuK?*…Õv¡?ïý"Ϫo?34¼ºE
?7ƒØÈF?34¼ºE
?ïÛ"×à?séí|Â3Ç?rn"	<?séí|Â3Ç?ïÝ%§Ã±?x~¨þ?qmpB§%?x~¨þ?ïùyÂ03??´@'ö?K¾ú.Žù??´@'öAGN4FGL J0252.8-2219¿ç‰ ­ŠfÀO£n.²À7ÐUÑì"À;¾t{'H@²«Yà@òþ½x?"Ð-'Å?¶փ¯Íc@ãrý›¢@XxPô4¿ÅÖSeª)¿áãА俿å¯>Õ'å¿æ—cÉÓô¿èâ­[µ³¿êªàHª"½AGNfsrq3FGL J0252.8-2218PKS 0250-225?ï÷ø•[$?k"¡ïbP¾?PÕnuc?k"¡ïbP¾?ïò¶a. Ø?\8~3¨@?Z"=;J0?\8~3¨@?ïãÒø•Ü?mšKná¾?l-ûÉü?mšKná¾?ïþú`Œn?9þY§FÕ? W+¨nDÚ?9þY§FÕ?ïø>y§$¶?M¢HFq¹?Oå·ïs?M¢HFq¹?ï˺°'/?"ö|™d²¶?z"§ó@(`?"ö|™d²¶?ïégÿ‡xô?q°^Ö¿à?f˜¶`3?q°^Ö¿à?ïüJ¼øÕ?4ÒXjí–ô?;•ª`Ê­a?4ÒXjí–ôAGN4FGL J0252.9+3834¿ïÝê)L;À2ipÅdùÀ:[>¢Òþ?À<YNÛʗ@Ïa&
««@%Ä'â?Æ"?ÃYí\9fÔ?öȍ$@Q@àÃA]ÃU¿á¤1£:á¿ä´|ÿ…ä¿èE¢>Ù°¿è3ªÇÜ£¿æuI"ˆÁ¿ïñ$€	AGNfsrq3FGL J0252.3+3830B2 0249+38?ïþV¯gŒ?"°cx	L?*"Öº¼aY?"°cx	L?ïõ
õ˜?Uñظ¦ð?UÇãŸÈ?ô?Uñظ¦ð?ïêõŸÝ^?b²I3ê¯?e
_æ(Ã5?b²I3ê¯?ïòïu»\?BQٛx%0?Z!u¡x{?BQٛx%0?ïý£nÚ~;?/¡Xý°?2ä‰úÃq‹?/¡Xý°?ïÐI'«"?}
P»'@B?wÛl4Í
a?}
P»'@B?ï´ÝþV_?x
Î	æÆ?'È€v'Ê<?x
Î	æÆ?拓*Ĕ?sæ
àó0H?…ß\.o£(?sæ
àó0HAGN4FGL J0253.2-5441¿æ'
Ê ¨ ÀKR.±Ä2ÊÀ9®æb IÀ<†Õ™úèi@È܏ú‰@åZ'"Ã?°uuøՔG?°óéœ;_}?ø=Žkh-ç@¯³ÏzÒ¿ÛN0¥lÕ¿árç]ò¤x¿ç»e4Ù¿éIiÀãàe¿æÇ>îRX'¿à÷ÍaGBµAGNfsrq3FGL J0253.1-5438PKS 0252-549?ïÿ`"
wc?$'&É?ïvÿ¡–ï?$'&É?ï÷fþ*¬–?Q‡ŠýºJ}?Q2`oDô?Q‡ŠýºJ}?ïòEK}p³?YãÚWgV?[ui3ÙJ?YãÚWgV?ïÿÑ[t<_>ëD¯‹ˆž¡>÷R<…Âõ>ëD¯‹ˆž¡?ïÿ›Õø´K?[¦Ò'H»?	
€'¿¸»?[¦Ò'H»?ïÜb,¬°?¡ëÛ¯`z?qÎé·³ì?¡ëÛ¯`z?ïç"[€?qœÈ ‹Ré?hâ{™+q?qœÈ ‹Ré?ïÿ™á)"?Ïö׳ò?	‡À!`
?Ïö׳òAGN4FGL J0253.2-0124?æµ´Z@ÀI‹Z ÝÆÀ:s­<
ÍHÀ<xåÕ²Nœ@׫¤^º@X¿ÜúAz?¾1Ò55?ž•AÆü?â^˜?ü4'g"#?焝=èîÁ¿ÀÆïh-:÷¿â·#\=¿à"Ñ~7hw¿ä	ˆ>þB'¿Ñ6¯ÿâxÜAGNbll3FGL J0253.0-0125FBQS J0253-0124?ïû,–r.?<'/äÇ6µ?CóMܤJä?<'/äÇ6µ?ïò¼êÀ?[Ap^öÿ%?Z†ü@}R¢?[Ap^öÿ%?ïð<6£;j?ZYnŸ®Ã?_‡'φ«¢?ZYnŸ®Ã?ïÖ¶²¦}O?Y¯/¤þ'›?t¤¦¨¡Ðo?Y¯/¤þ'›?ïóþy?K#Ãàae?XwÆñÑ?K#Ãàae?ïÆëU'È^?"«õ‰%û_?|ŠUGðó?"«õ‰%û_?ïçmL+?t³MÕõ?h'³èw'§?t³MÕõ?ï]A¡Wu?|Kì?"WËÖÉ?|KìAGN4FGL J0253.5+3216?ï°yTª§3À7ÝÝãu…¾À:LŽ¶È¥À<VU°5½Q@°uÔ@9D$>û?»
Äv)?¢äž5ñ»?ç\V­‹¾æ@N;Qkƒ¿ïý‰-:Ë®?ïÿËA²Q÷¿åü&¡ÕRW¿âå`w9¿Ý-` Ô¡W¿äƒ«ñŠòAGNfsrq3FGL J0253.5+3216MG3 J025334+3217?ïÿE›?ó,œ9Ù?]¤Õïaô?ó,œ9Ù?ïö»Y?TËöÍ¢Ü?RzzÙά?TËöÍ¢Ü?ï–¡m?mÆ'‹…?aTS|œcD?mÆ'‹…?ïÿ¶"&=,>ð&Ê*zœ?Zéõ?‹>ð&Ê*zœ?ïÿe‹þ"?Om 
L?Nw¨NV²?Om 
L?ïÙ~"üdÑ?áâ'?µÞ?s@½h`{"?áâ'?µÞ?ïð+âÿ6?n#拦?_ѧÔM%I?n#拦?ïÿcˆ®t?r7	Ó	W?ŽýàÚ­?r7	Ó	WAGN4FGL J0253.9+5103¿í‹KßÁ5À¨—š¼À96Fñ'À;̯,¨Õ@Ä7B·`@‰Y_í¦a?±Q
¸Á?¯†ë8üv?úôš ¨4@×ÒÙ+Tí?înŽ¾tDu¿à7–oB­ú¿è"ÆÜ	¿âù'žªz'¿éI^]®[ó¿ïÖýÓ*	AGNfsrq3FGL J0253.8+5104TXS 0250+508?ïý»õl²?O;þYöC?7ò"Ozi?O;þYöC?ïóÙ¬S?buæÉ鑫?XL§ÇÞg0?buæÉ鑫?ïå³ÿT-?gYÊ,!±­?jL©/#-?gYÊ,!±­?ïûöZ‡,|?+'ë£^?@&•wÆ÷?+'ë£^?ïûÆñ¸â?@¯ L'T:?Cüä´A«1?@¯ L'T:?ï¿[ H[?Žî9Ùën?€)7êyœS?Žî9Ùën?ï£ÍÑì1?‡eƒÄC‡?‡‹¾4œ?‡eƒÄC‡?ïö€"}?DBëï"w?RÿÑÚV?DBëï"wAGN4FGL J0255.8+0534?ëTìqíÀFÉ2µ^ñþÀ:½âïÙÀ<K4-@&ž'a™£@Ø8 þ?α^œÃo¬?¼µ‰9O,
?ñ£ø,Ìç¥@ªdSç‰?ҍyYˆ¿çCÞ¡¶sš¿áå­é¿¿à°
fóT¿èžP¸7ï¿è­ŸÀ¥!7AGNbll3FGL J0255.8+0532PMN J0255+0533?ïþ?©
Tý?(~º‰Oš?,nЮf?(~º‰Oš?ïôØcG¼Ç?ZÊ}&CN?VO9ôwq‹?ZÊ}&CN?ïñð"–ê,?f²QÏ+?\Öqö™M?f²QÏ+?ïõÚæH§l?6Ü~þnd?TJ3š¬'2?6Ü~þnd?ïý75¡L–?1}°b'€?6FRGâAG?1}°b'€?ïÕEp'Qe?€Oä»H{?u]G·WML?€Oä»H{?ïé‰d©^?v	cí—rû?fv›`@Îü?v	cí—rû?ïÔ&#fr·?cÚwU…?uìî<øp¢?cÚwU…AGN4FGL J0256.3+0334¿ëÚ¾¿EªÀG}BÙÏÀ9÷íPÐÒìÀ<AåçP@Äþ¹®â×@"2A›«Ã?¶Œµ°{ˆ?'YÿáÞ=?ÝG!&Á4é@	$¼¥BÉ?ïû†ô{g¿â¤'ýuE¿ãÖÂ^ß´[¿ß3Žµâ¥¿Õú}¹©"¿ìÒ¯/-5AGNbll3FGL J0256.3+0335PKS B0253+033?ïþªxö8?ÒCvi-¤?%Xn¾Ùn[?ÒCvi-¤?ïö¦jëäÉ?R¦L{jB?R³)ྏ$?R¦L{jB?ïøºüÉG?QßÎäÉ«?OÑÏwô'?QßÎäÉ«?ïý"çé§?"¤ôñn?6èÆÐËÓ?"¤ôñn?ïýë¦Û?&g‡äÈAW?0¢ÐWµöç?&g‡äÈAW?ï×ÙbÝDê?€¤|ÿ"D?tN {Òá?€¤|ÿ"D?ï÷Zª‰?cáôÌM$'?QçLGÞ¾J?cáôÌM$'?ïùÀuÑhh?92èÖ-ø?Hþ)Rì-?92èÖ-øAGN4FGL J0257.0+3358?ïè.ž	ôÀ6K<>t°À;ëÔÏÑÀ< ˆÛ¢@ Qg¢P¢Z?þÊTg`aj?ËY
Þ*m<?ÄGøý'LK?øz_\†é"?úW|5°'?ï'سiy¿îký^åé~?¾Ð_("ƒˆ¿àEéÞö!ÅL¥Ë¿çžÑ'ÙAGNbcuGB6 J0257+3357?ïý<Bó¼ó?/PÑÞ+Î?6æ‰N*U?/PÑÞ+Î?ïç"ä'«?j«®¨9ç?hl¥®•÷?j«®¨9ç?ïêÁ×ü*Þ?\Õùô.¯Ñ?e>(	T¨?\Õùô.¯Ñ? ˆ³?j!¡X\dé?ŠÚ—Ýú#?j!¡X\dé?ïû%T>?<j§1®Ñc?Cj°‹é"?<j§1®Ñc?ï"/›ŠEÐ?'·û\ì»?‹4T?'·û\ì»?ïՍ~`á ?uÁ9ø—ª?u9@ï+—î?uÁ9ø—ª?î›{­0¶?˜$•™Vi?®–HFۘ?˜$•™ViAGN4FGL J0257.9-1215¿ã_N5(gÀLmîËûµÀ:6¯-•À<tÞë³Aá@ß?@1É@oœp
¯?¹Þ!
j¢?"h|ü*?ÕåFÁ/Š²@Õw®bS‡¿Úƍ«p¿å¯¿üò¿è…xDµ;·¿åP½Š'¿êšÏ>—"¿ïÿ€^	J¬AGNfsrq3FGL J0257.8-1216PMN J0257-1211?ïý•?þÙË?%dÒãYî#?3Uÿª¢ËI?%dÒãYî#?ïöa…£dì?UÎÒ:¾Ð‡?S<ôß±È?UÎÒ:¾Ð‡?ïêì=^
?\eŽÓٍ¦?e–ä?\eŽÓٍ¦?ïÿ.Äcœ²?$¸ß3R¡?'q~hK?$¸ß3R¡?ïþž3ºË ? ¤ßüéͧ?&ÁÁËóô? ¤ßüéͧ?ïÞ{'×ês?ru?4WÒM?pÂ6ù=Òt?ru?4WÒM?ïñSŸJš?c
ù4Š"e?]ÍXÆê,~?c
ù4Š"e?ïý•"wµT?)]ۙsTÐ?3VêβѬ?)]ۙsTÐAGN4FGL J0258.1+2030¿Ö¾»^‡ÂÀ@ªé>›AÀ:k$-ܲÀ< p­E£@x¾'²!?ÿa­ê‰v6?Äðª7 ¨—?Ïuéüˆ|;@WÚè'®@	úâ"tt¿ïþsÙ°k?ïîQs	?À#^~æe¿á­:*ž9<¿æ¾J''?¿äûF'+½ôAGNbll3FGL J0258.0+2030MG3 J025805+2029?ïúÃ|ZÞ7?:7`JôN¼?Dòn…?:7`JôN¼?ïð D6Cg?\_¡b%8?^¿wu<£?\_¡b%8?ïÚFÒGe?p°`²&Á?rܖãî'Ã?p°`²&Á?ï×}:›åØ?Véό!»V?tAbÎ9ßú?Véό!»V?ïö^´ã™?O³ÅZ[L?SãClœ¢?O³ÅZ[L?ïÍ T3^?}é¾+"'v?yxïð³DÝ?}é¾+"'v?ïA±äq·±?û&z³½l?—ÉÃz`Ø?û&z³½l?ïVoÕ>Ð?"Ôкï?•2X%þ9?"ÔкïAGN4FGL J0259.3+5453¿é'J™x®àÀ¡!MW¢À:Œç='[À;́I@»²@ ¹zæ{¯@È>{?«¡ƒóÀ¿¦z¡÷Ùb?ç¥F`Œ‡¸?ñê2]ö*i?îpÿ¡á;Å¿ãçOš¿ç}îãx	ý¿ë‰ÝÏSÊ?кý Ë¿ßÎ59©AGNbcuGB6 J0259+5451?ïÝ<ñoeá?"ÿà<Ė?qa‡iù;h?"ÿà<Ė?ï·ÓÈáÓ?ïÄYÙ?'
Nj;Õ?ïÄYÙ?ïgdڎñ?Õ–¨§?"d¯Ù¬A?Õ–¨§?ïÙá4…:3?bôŠ:ÌE?se©u*_?bôŠ:ÌE?調(ڄ?‰Ø…WÛC?…Q¹òYÃ#?‰Ø…WÛC?ìÆÑÐd(k?ÁúÜC|r?¹Éq|Þ¼¨?ÁúÜC|r?îðœæ o?—v%›üèw? ö?ÏD?—v%›üèw?íF½L.?°}eIÝxÿ?µÊ>·«?°}eIÝxÿAGN4FGL J0259.4+0308¿è*â-uó¼ÀGbŒ?>qÀ;zVÞ3'À<¸ÁDŽP@"uE?¥1}?÷è»ûÄ1?×›Á''?Áº	戶?ê&¿AžÛÎ@Œú–Àn¿ïÿ`Ï‰@?ïÚ ri¿ãÛJ¾ëԿَK½m´9¿×QmZ÷Gu¿Å^eYAGNbcu1RXS J025923.7+030736?ïÿ`ËûI@?Š‹v\ù?æx
Ì?Š‹v\ù?ïõ{|Îß?W(>k€@ª?U	tpb¼?W(>k€@ª?ïð%‹%"?g¾o:ðÔ?_´éŠk·?g¾o:ðÔ?ïýáÿB?'Ôª4gK?7GÂ?_ÑI?'Ôª4gK?ïÿLa‹÷?Fë':?sÍíµ*ê?Fë':?ïÕ1èxá?xù¬Üóݜ?ug~›'Ãn?xù¬Üóݜ?ïÝïò–µä?~MI[å?q±å]Å?~MI[å?ïô¬¨üZ?Rþö/9±?V¦­ïš?Rþö/9±AGN4FGL J0259.4+0746?ë®é³žŽ²ÀE¨×¾˜V£À8¦ºò¯µeÀ;—ïrBÓ@qieŸA#@ùü£T-?¥½'&?¯Äà^ô"@	ž>^à`(@:ÍûXü?ëÄS­úпÞϸ$B`¿ã1¾Ý`™¿âgM"—¿åÈ×tÆ{z¿æª ¥gAGNfsrq3FGL J0259.5+0746PKS 0256+075?ïþo垳g?Nr¡Çü¢?)¢Oj€…?Nr¡Çü¢?ïõF€Š²?Z5HØ},k?UsîÛ.«4?Z5HØ},k?ïîm~Ľ?c"¼${è?aý'—8œ?c"¼${è?ïÿ
Ëq>B?¶ç"#™d?¦'‰
Ò?¶ç"#™d?ïþZ÷¥ñõ?#‹ìýv?*P'šÒJí?#‹ìýv?ï۝ÿž ?vÒ²x¸û?r1Bââ?vÒ²x¸û?ïâIÖã§?r×3ˆæ""?m¶)(·"	?r×3ˆæ""?ïþNè†? …L	½å?+€ñì£]? …L	½åAGN4FGL J0259.5+1924¿ïžÊü4¶ÀAÒܱF_À:y–°±
TÀ<#/V/@óôëû@õ
3¿?Âwÿk±?r§Î2s?°nD_÷7?ü€íÑ)Rà?ïl¤nò¿ã[QàG}î¿æ››œ©"¿âk
=²é¿ê4:WÎô¿Ýe5#xU&AGNfsrqTXS 0256+192?ïóÑA^?OA†ñ¹?X]~^øWn?OA†ñ¹?ïñÁ÷KÀ?`NÁå®<3?\|$nØ?`NÁå®<3?ïÍ+TA ´?yÈéiÃč?yjUÖð•ë?yÈéiÃč?ïÏ£Ö«À/?Zí4öŒ?x.°ÿ c?Zí4öŒ?ï½ Uq1Ø?uÀ¤ðl¾Š?€·êª'Â
?uÀ¤ðl¾Š?ïÇ`±ñ4?"–·º?|O¦ô–<?"–·º?ïq*¼¹{¯?»‰ÏU	?'Ú¨c© 4?»‰ÏU	?îôQ;e?…cê`0—? ºìL/]°?…cê`0—AGN4FGL J0259.5-1705?﬌…m¬ÀMcðí=…À;,>׬#àÀ<ªçcQ0@ Ò{ÿ)ì8?ùâwXüñX?Óô¸#G'Ë?ÙAŒ&êO•@¼[ed?þoKº">?ïôGe_M¿î½8À:î?Æk¼f£".¿Óx‹A'¡¿Þx'}sHL¿ïçB.x¹OAGNbcuNVSS J025933-170540?ïùg»â*?A5.˜är?Ja|®J?A5.˜är?ïé"%q²?j/( +?fó{Ã0õù?j/( +?ïÅ'ØÈ>Ú?q K½€B?}l…3'??q K½€B?ï©ýuÈ?[?l¯JNŽs˜?…€¢"ÏaP?l¯JNŽs˜?ï÷O%hU?R=T$"'Ì?Qa´¨¤0š?R=T$"'Ì?ﻍZÈù?ƒœ*‰¾Ÿ«?¿¦æ­?ƒœ*‰¾Ÿ«?ïÐó¢pû?z(ñDE?w†.·Yó?z(ñDE?îæ:¯Sj5?'7­¿Œ	ž?¡œU*¨?'7­¿Œ	žAGN4FGL J0301.0-1652?óºÀM-«KrÅÀ; g4À<€îßFL@xƒ/ö@A›@bƟ?Í@›üu[ø?§ê­ÞJ"¹?à÷¦ë@šÐ"Øi¹?—ŠØ>M¡?ï"=ý'·¿çU4_ƒV¿ÝRìÁ´À¼¿ç+=e¼{¿ïúª@/ðÞAGNbll3FGL J0301.4-1652PMN J0301-1652?ïÿØù	?™4
''?½Æ_€7?™4
''?ïö±ëíF?Tøm®¯?S✞X›?Tøm®¯?ïðîÎ̤?Z0·>Û\?_ô"æW·ö?Z0·>Û\?ïü¥ôW™?#)ëD\Õ\?:Ð\"BÊP?#)ëD\Õ\?ïþúö$ý? %ðþÚÁ­? PŸµÌ¨? %ðþÚÁ­?ïÕÐV¥6?wšewK6š?uÕIÌÀ?wšewK6š?ïÓü­ÿÆä?}ÇÑ¥£Œè?v©,R?}ÇÑ¥£Œè?ïóÊK#{?Kòª"h?Xki'@?Kòª"hAGN4FGL J0301.2+2546?æè}0ÇÀ<ŽDR?gõÀ:ö} >ÏIÀ<dX£/D'@ÿÜ0B@ïêÄ.˜š?ÇnšgtÙF?§±U¢ô·"?àÊzw•bÓ?þ5&U)R4¿ç™ëcÉ?ê>zúr!†¿ß)ùc-Ì¿èiU./¾4¿âG)T ¿«-£SN(AGNbcuGB6 J0301+2546?ïþô¿ì%?!<9¯ÑJ?.°³ñÙ/?!<9¯ÑJ?ïójvI?X…ôÕa<L?Y+ÃÇ?X…ôÕa<L?ïçýÞEMÆ?YcW"A»?h!Þn*@?YcW"A»?ïåÿRõ}?PyŠ½'ú?j­ÓL´?PyŠ½'ú?ïú«¼J¸O?@ý#Ô?EQ&{ê ?@ý#Ô?ï¹6£*<?ˆÉÜ:O|?ºrg¤å?ˆÉÜ:O|?ïã"綈?qæŠ]›wy?lÝ,›6K?qæŠ]›wy?ïWT+6 ·?"fû²Ìo'?•z—t?"fû²Ìo'AGN4FGL J0301.4-3124¿ïë¬íšˆéÀN¸G¡A)À:ÉŠ ÒÀ<¼¨¨*V@áÚûä'@/S6L?Ã]:ƒ3¦¡?±ÒIäO Q?ì¼^'í0@QºÝ·¿Ò=?%¯½¿Ñ@{EE¯b¿èe¥@–É¿ÓüνgÔû¿éWÌÊæn¿éõF2ê8AGNbcuPKS 0259-316?ïùµª‹D?L}T¥Wíš?I)ULÚA‰?L}T¥Wíš?ïóÜ.P¡?Z×®)¬ø?XG£Nl~<?Z×®)¬ø?ïÖ¿^†?pã¹ßpy¡?t Pîáç?pã¹ßpy¡?ïò1.d?A©ʦkx?[ÅÔ²2»?A©ʦkx?ïêßʘ4?b¿Èìws?e ;}eK«?b¿Èìws?ïѦ"þEÚ?,}"¬?w,½e`2ï?,}"¬?ï¾Ú~Ä´®?'¡–Æ\–?€I`Wäv?'¡–Æ\–?ï¾L'?lܶFœö1?€{ºò=úS?lܶFœö1AGN4FGL J0301.6-7155?á÷IF+C·ÀDã[ÕìlÀ:"ïÙAOVÀ<Š³Ï¥Å!@'ñÒjÆr@óÕ4z[?¸a=݆.?°¸9þå‰î?ô+¸e6»~@Ÿ®†¨?Ðt=$à¿ã4ÿ@'lT¿åf‰l$ìI¿èrNf•`O¿ì°a¬m\¿ïðȊGìÿAGNfsrq3FGL J0301.8-7157PKS 0301-721?ïý%¿¤'"?;š¸Å°þ?6ÒDÉR‹?;š¸Å°þ?ïöÝP
ð•?S>¼ç?RE`ØF=?S>¼ç?ï扼#Sº?r¨÷C7Ÿ?ivCܬFx?r¨÷C7Ÿ?ïüvA6p?(aÉj¦X0?<Mõ, d?(aÉj¦X0?ïûßù
©?5ANÑþ?@€å'?5ANÑþ?ïÞ0j#ç?}b~‡¿Ü_?pçÊçàȄ?}b~‡¿Ü_?ïês¬A‰?s‹fPÆî?eéŒtº¶y?s‹fPÆî?ïóÄÐÔï0?M±·Í«&Ü?Xv]â®ÀX?M±·Í«&ÜAGN4FGL J0301.9-2731?¿%'ƒŽÀNŠó¡LìBÀ:©·¢åsÀ<°XaÀå8@-^g¿Ví@ˆÐâ2?Å.ä —?»œ©'ý?ö8›P˜Ÿ@3êrúôR?ï¬W¿ãž"Ô]ºÆ¿ãÓÂT£ÆC¿áÝŸ¤u–¿ê2ËŸ¿ïÿ3Qf$!AGNbcu3FGL J0301.8-2721NVSS J030158-272754?ïýxEƒdE?&Ü?¡H~?4=Õ;êÍ?&Ü?¡H~?ïõ¨3÷dŒ?Tôl²[‹…?T¯˜n¬G%?Tôl²[‹…?ïêáWÉ?¥?hՍª¾Ö"?e¨¤"®?hՍª¾Ö"?ïö§áØ!?8«±6
j?R°>H=I?8«±6
j?ïý~™Ê'<?0Ðt­ü!?41¯ß—–?0Ðt­ü!?ïځëŸm;?sàÍï,?r¿
%úŽÈ?sàÍï,?ïãùó?yK¢‡«7Ø?låì	$UC?yK¢‡«7Ø?ïã+¢´å?X1…nùaÈ?lÔ]f—Ì€?X1…nùaÈAGN4FGL J0303.2+3149¿åç[=ŠÇfÀ76˧2ßPÀ:hµ}$îÍÀ<@¾(Å@tÙrÍ|ö@i=Š¥
?Å-h±Å4?Än³&ˆì?ÿ»iGÂ6q?ÿÿ—ðw ô?爆ìî«D¿âÁ²‡§(οã%Ɉt®(¿æj}ík¨Æ¿êHuà+ú/¿ïÿùëñAGNbcu3FGL J0303.0+3150B2 0259+31?ïÝ:Îæ‹?lzfÔòt?qb˜qí€f?lzfÔòt?ïÇe­y?|¬u°ƒ…y?|M˜D7›?|¬u°ƒ…y?ﬤ2q8Ê?{³~‹åì?"ÖóUó]¢?{³~‹åì?ï}Þ?x†úNõå?Ð]Dš(?x†úNõå?í鞎‹t?¨£Ø}S>¡?°³
±eà?¨£Ø}S>¡?îÒÿµò­?£HÂÆÌs?¢ÐžL7?£HÂÆÌs?í¦0åÑ?¤>Y¾˜¨?²ÏOž
Ýù?¤>Y¾˜¨?éâ{·JHg?£$Ÿ´ 7?Èv"ÖÞb?£$Ÿ´ 7AGN4FGL J0303.3-7913?í…U§ÞÀAý´þyîÀ:F‹yEf<À<c@þÍÐÙ@rË7@‡¤¤—?½ù
†? Ç†>?ã	Õ×7‰Ú@
€«Œ
e¿Ñÿø^¿ä"\0ýN¿égþìډ¿Ù@ÛýÂ8¿ë¾Ïÿ1N¿ïÿLkAGNfsrq3FGL J0302.5-7915PMN J0303-7914?ïý`°Íp?*µíâ6H?7ôü´?*µíâ6H?ï÷>ts´?S»êj'*î?Qƒ‰Jø:?S»êj'*î?ïì¥cëü'?eüZŽSÛÃ?cZœ7¿n?eüZŽSÛÃ?ïý4ók‹Ù?!Í[ôGI®?6Xdi[€?!Í[ôGI®?ïü¼½ú»·?1B=ÄA9?:zeòa?1B=ÄA9?ïÜÛ"P?t;«·±æ?q'n½Üôª?t;«·±æ?ïî'hçŽß?rj*=Ý°?am–à‰Š?rj*=Ý°?ïõ¬€Îõ?Ei±ïæñ?T§c•å$?Ei±ïæñAGN4FGL J0303.3+0555¿â¤æ¼ž=ÀF-û¹À;Tšù*4À<‹ºˆ&ª@"¡ûï»?øÿø¨ó©°?ÖwºKÀÉ?µÎî:/Ѫ?âºcslß&@bü]^*?ìÈK~ºE¿ïÿòß0&¹?ïþ'¨'Y¿ä«­Bm㳿¾Ã!¨FZ­?‰R Ð‰^¨AGNbllGB6 J0303+0554?ïþö^ÿ?·—ˆÅÚ? Ÿü€Ñ0?·—ˆÅÚ?ïöMHL
ä?Tˆ–&q}¢?Seo²ÆÝ?Tˆ–&q}¢?ïïÖiP?aßÁÂü–?`)–à ´ª?aßÁÂü–?ïù7TçC??•†c>u?K"«ß	8"??•†c>u?ïÿ7i^ús?Ô{¿w"?Ûú)YÊ?Ô{¿w"?ïØۙjZ?tq=_}P?s'3_-+?tq=_}P?ïóGFªM5?d)æÓf†?Yqr7ò¶ô?d)æÓf†?ïðÆ$Y§?X¸²óãŠ?^sӦΒø?X¸²óãŠAGN4FGL J0303.4-2407?áOòÉ-'xÀNŠ›ÏÔ¿À7¤¿Ä¦ŽÀ;'­¯Ñƒ@g½ml
?ý"«þöë"?•p³W–ûì? w›ºR™@<ï>çœ\@š'ျ¿¿u š"¿×ö‹ÂÁ[*¿ß
X^©¿Üª½"µ·‡¿à·4µs¿Ýìðƒ¶-yAGNBLL3FGL J0303.4-2407PKS 0301-243?ïÿ	Kiq?PX•¿Ü?þÛC|‰?PX•¿Ü?ïöÙO*úC?S9]Ÿ8"?RMaÂÈ©?S9]Ÿ8"?ïä—Tx…Ö?sõÝW(™É?kh«ºTan?sõÝW(™É?ïÿ͎¤Ú&>ðç&ª¾î–>ù8¬±¿;>ðç&ª¾î–?ïþÎ]? Ɏ— b?'ãÂÚY? Ɏ— b?ïÖ&dà?ÕòO
:m?tìÍØïO™?ÕòO
:m?ï笯ÿj7?sÑ©›éVÑ?hSOåéž?sÑ©›éVÑ?ïÿÑÇæç‰>òÏæÐí>÷+Эræ>òÏæÐíAGN4FGL J0303.4-5232¿ã3#¸ØqÀKVx|é_«À:NÇw"vMÀ<mÏt@3ÏDvQ–@Ð"<jêZ?ÄE¡Iç*?ËЗ;ÊÜ@c±€@,@@rwÅç«¿â\^¿âⴕžbV¿ëf¿§ C¿é©Ì·ÔD¿ïþÒ8F˜k¿ïð®SeâAGNbcuAT20G J030328-523433?ïøž<¤?G)‹s…?Oé‡S9«2?G)‹s…?ïötÏÆãe?V[~ÒS)Š?S`@¾ÖO?V[~ÒS)Š?ïÃÿÄ?tûf–ùˆm?~€j%ê?tûf–ùˆm?ïýMa÷Z¯?$òÙ#±þë?5"ðis6º?$òÙ#±þë?ïùÂmDÉ?HeB¾4?IÈö–Ê ©?HeB¾4?ïàæ7Æ°?q?›¢c'Ó?oúƒ É?q?›¢c'Ó?ïxúÃU?ˆºÏ2þf?þý%ÎÿT?ˆºÏ2þf?ïóE'"?O²ã*?Yuæ€	ø?O²ã*AGN4FGL J0303.6+4716?ìk-†SŸÀ#µx_.QÀ8rÆ	d,ÐÀ;˜äXڌ©@ˆƒÇ =@Ǧ†è½?¢§û\,PÁ?´Qç¾Àš@H<¯³·@Ԓ¾Þø?ޛà»íŸ¿ÜŸF¡úç¿âŸA¤:¿ã=OK—®¿æЎÞT´¿àíñ_©2êAGNbll3FGL J0303.6+47164C +47.08?ïûNŠüs?>NÕZáo?BÇ­¾´À?>NÕZáo?ïî]<t0?hUHéÌ4"?a¢ÃöLÀ}?hUHéÌ4"?ïÚÆ«S3?xåp$ZÉ>?rœªIWöV?xåp$ZÉ>?ïÞF¸(Ùq?VU±ñªÖÇ?pÜ£ãT7¸?VU±ñªÖÇ?ï÷"B8ù`?Q÷Aµ?Q»{\'á?Q÷Aµ?ï–; êñ¦?›\Twþ?ŠqÁÓú‡?›\Twþ?ïž'ó¦ð?ß&â/$?ˆ{CCþ?ß&â/$?ï}]¦yPú?z'ž7?Ã?TK/Ê?z'ž7?ÃAGN4FGL J0303.6-6211¿é—«OÏvÀHYå\ËOÀ9Q³ø^KÀ<êg¹M@¨3vë@Ùb<5:?®É)¥?¸S´²ú"¯@c¤%
×@‰ˆ)"´¿ÞpGÛá½ ¿à6¹?|AÅ¿æªiËuµ¿äZTª|?ì¿ë(ÔɎտïþ²í'¶AGNfsrq3FGL J0303.7-6211PKS 0302-623?ïü­á¶O?00¼.ìZ?:ñâà,&?00¼.ìZ?ï÷-J)ސ?T6éߡͅ?Q¥l2ó8?T6éߡͅ?ïß¿ë_Vt?eÕø—T"?p 
0r?eÕø—T"?ïÿ'ûÐ#?;hè?Û`øÌ|?;hè?ïý{ûÆVÞ?*}'A=??4 !îEM&?*}'A=??ïßNñ™y¨?qyõõÈ$?pX‡" ?qyõõÈ$?ï»Éù'?'/ê?8zEšµ?'/ê?ïý'Pau?.óÒÉ+`?6Ç=!±ìE?.óÒÉ+`AGN4FGL J0304.4-2833¿ët¨úýžÀNU<æÀ"À:øÕ!/$±À<˜5¤&»V@! pe˜¶?óV¡—"Ü›?ÙÃp,¸Å¯?ß(Ì|ðÁt@j¸A$@eK#É3?ï÷D9ë´?ï¢.(1wq¿å°'b"s?Ë´¯¼пݳÿ¡`bk¿çûûŽ7£AGNbll3FGL J0304.3-2836RBS 0385?ïú=¢Öb?G¼Â•4B?G·	6‡"ž?G¼Â•4B?ïìËlœØ¶?eŽc_¿¼?c4"3'?eŽc_¿¼?ï§Åi+<Å?ؽ]¦sÒ?†¥§r^è?ؽ]¦sÒ?ïυ<¦Šª?eº‡t®Ë«?x=ašÜ³?eº‡t®Ë«?ïôžö?V´t'†,?VzÃ͘!f?V´t'†,?ï¶äŒËÄ©?‰Á»{àƒà?'FÜÏ™È?‰Á»{àƒà?ïœct³J	?Š/bMñH?ˆç"àëíÃ?Š/bMñH?1YÙ?…¤þ°'X<?¸"w%¼?…¤þ°'X<AGN4FGL J0304.5+3349?À¦—®ÝÎ}À5\ÂÅâÍÀÀ:ˆÝÇÆӏÀ<ڀ¶–@ò1Xèy|@æΆ
pœ?Õ
å=‡?؞œã¦3@_¶™" ä@%#ûݱ¿ìºÁ5¿Õ?ëAµ!_v2¿ê»à¡¿éáìžú+«¿è²2·ã0¼¿ïéXü˜AGNbcu4C +33.06?ïõ¬y	?[¦Ø,`Š÷?T§
ØBñ?[¦Ø,`Š÷?ïà/!™ô?vL…2s?oÐß_Ëè?vL…2s?ï$uïà?'ªWŠ‰?ŸqBýÞ?'ªWŠ‰?ﯓ%-®[?kZ_t³?"6'n?kZ_t³?ïçTúrW?x:´Oö?h«qð¨?x:´Oö?îÀJv¬ëÂ?¹0¦—?£ûX˜ ßÚ?¹0¦—?ím*Ü	£?£R…÷ºÜì?´–¯ËEte?£R…÷ºÜì?ëf5ºÄY?°º|NkY&?ÂgÏ)îœ?°º|NkY&AGN4FGL J0304.5+6821¿î!-ræË@!.Ÿê$ÌÀ8Í~¼ž`À;SàGÓÔ@^^ߎš@[\|ؘ³?°­xH¼?ËK­h¿@U§L	ÃÎ@H®ÅzÉ¿Åçû;õún¿â½:ZMS¿èXžâ¿éÄÜޒÇî¿ëyóa2¹¿ïþú¡Ç:'AGNbcu3FGL J0304.9+6817TXS 0259+681?ïX(5(Uà?"²'ðÕV
?"úùW…¨?"²'ðÕV
?î«-#a?²b: §S?®õM$šô?²b: §S?í'5&ÓSz?£Í±×±ŠÛ?³vVÉÓW²?£Í±×±ŠÛ?îVÍiËg?ˆ£Èz5XÛ?ª")krå‡?ˆ£Èz5XÛ?睨\¼?Äù|&Ûл?ÐįóßFˆ?Äù|&Ûл?â?¸svx?ÒÕª¥õ6g?ۀŽÅ?ÒÕª¥õ6g?äönØaÍ?»º«?Ö"O=Þf?»º«?Þ6»(	´?¶s›>ނÅ?àüd¢kû&?¶s›>ނÅMIXED4FGL J0304.5-0054¿ïßAº=0ÁÀHXǟfb5À:â,[ØÀ<žBuÆ@Ì0ÐWpÕ@X϶¤l?Â.ú(ûvÙ?€åƒõ9õ¼?ÀqU­±~"@³>†MŒ¿ïû–ÿ‹eú?ït¦Àž–.¿à(é}Ý{q¿å
*Ž:Á¿Ü"±þ?`"¿Ê¦2™°?ÎAGNbllRX J0304.5-0054?ïþ¿UÀÑÂ?¨-²,¬?$
¦\Ðҗ?¨-²,¬?ï÷mûÓm?S§{҄×Ì?QÁ#še¦¶?S§{҄×Ì?ïñ™ù;?OZ›¬bz?\Íù±Õû?OZ›¬bz?ïý\^r¡? ´Šôo'j?5 H$? ´Šôo'j?ïý$dÓ5?2'ãm¦t?6ÜØÿz9þ?2'ãm¦t?ïعkµÊl?uL
NžWÉ?s£J
MÖ_?uL
NžWÉ?ïì	ËRE¿?pt¬ßKqo?cö4ºØ{?pt¬ßKqo?ïö˜Ëhs²?E†£îyÜÖ?RÎh»¥¼ù?E†£îyÜÖAGN4FGL J0304.9-0606¿ï¯K½BÁÀIû5ü;OaÀ:´BˆCÀ<|vOèu @Þä^9@æCåÍ?ÊÅ4'$E?¬nÊcª?à52F¤)@@â)é•ö¿âÄâˆô'¿ÝG­¾"¥¿¿â$ýh %¿äL<ÿÂ«¿ã_iG¿ïÿþó…õAGNbll1FGL J0305.0-0601PMN J0304-0608?ïþÐaúx?‰Àx÷Ê'?"ùá+Zޚ?‰Àx÷Ê'?ïöuÁ^jÖ?S"ù×ø×?S}Ä[¤?S"ù×ø×?ïò%,h"?\ÿLà†"¦?[µã ~)A?\ÿLà†"¦?ïýàûzV«?‡ájå×z?0ø%gÀ'?‡ájå×z?ïþЖ—ï?ú7Á·-4?"ö—îiÅ?ú7Á·-4?ïÜրæÖt?pSNÙc?q"¿…µË?pSNÙc?ïî0Œå¬?mɗ­¥?aÏsOíÐì?mɗ­¥?ïø¾r–öQ?>°?½AL?M4ç•Åõ?>°?½ALAGN4FGL J0305.1-1608?èoŒ·«IèÀL•!Ý Y§À:€'_ét£À<k7…¨K@!	‰Í?û€N¤¨ÁU?ªÄw=Ï?®. |wJ?îÚ³	­'ì@
þ"™Or?ïÆÛl6Š¿çµÞÿT^|¿×ÐPåË¡T¿à"H÷À–¿».ù<ÂS!¿à.ŽˆÄ_AGNbll3FGL J0305.2-1607PKS 0302-16?ïÿKŠË~!?s¼þ÷?Ž§À#•£?s¼þ÷?ï÷[Î×?RÑòN-3ç?QI˧f~?RÑòN-3ç?ïúUIïžo?4ƒùÊÏ:Œ?Fª×»bPé?4ƒùÊÏ:Œ?ïÿ
GöÐ?‰Å²ý¹Ç?W#ra?‰Å²ý¹Ç?ïÿFwÉM?
N	T‰8?1 ûUƾ?
N	T‰8?ïۘӲ*p?sÞlMVX%?r3–þL?sÞlMVX%?ïú0ƒwç?^¸"ÛºX?Gó>}6ûn?^¸"ÛºX?ïýäúÀûÞ?$´¬™»À¶?0Ø+Ÿpì"?$´¬™»À¶AGN4FGL J0307.4+4915?ïúZ"ÀGc€X€À9
¾.¤XÀ;ªQ­q½²@µ$h?ÿ	GŒ†‹ ?­Nçï'õ?¸ Š6Nœ@©ÊAR@ãTpšœÏ¿ánoês¦Á¿ÝÃT~–¿Ù3$º¼)¿âÎg öo³¿ß6#¨{µ¿åû¦Ôë?AGNbll3FGL J0307.3+4916GB6 J0307+4915?ïûuŒý‡ˆ?<…þ4=D?B)Ìàž¦?<…þ4=D?ïÝb幓ñ?p÷ý'ð0d?qN鳝?p÷ý'ð0d?ïÚ¨~Ӊn?v ·ÔmÚ?r«À¦	|É?v ·ÔmÚ?ïšÁ7ÿ[ü?hmíàjþÄ?‰O±òjù?hmíàjþÄ?ïë£×àý?düz}ŠEo?d\(;ß²^?düz}ŠEo?ï9•ìõ?§²`qÒ!Ã?˜Í_]¢aX?§²`qÒ!Ã?ïš…Js?Š!¾@ÂèÈ?‰x¯X?Š!¾@ÂèÈ?í¦K'_"9?˜6`Ò7KÅ?²Í¦Ä'÷;?˜6`Ò7KÅAGN4FGL J0307.8-0419¿Ç6€
¸{îÀI%ŽÉ[ÿÀ;`ØÞ¨—À<°yixiž@ÆðŒÅuÀ@ڒ_ét£?Î'
)¤"?xÔ â«^Ó?¨D<ߞ$ˆ@åGÂâ=?ì©ðÿ±üg?îâBµ‡5ê¿Ý‹@»\¿Õp^aàÜ¿é'Àoz¿´ŸEÀ~ŠÊAGNbcuLEDA 095522?ïü¥×¤?7S^TŸæÇ??ÚÏoªš?7S^TŸæÇ?ïözÊîȘ?U!iÒėü?S
iàvQ[?U!iÒėü?ïá–æ`ò‰?kÜÎY¸*Æ?ni‹Ï¦ü?kÜÎY¸*Æ?ï÷ßpχ#?7L>wéú?PAÚA±?7L>wéú?ïúÌ@y±Œ??ïp#="?DÎýÍèÈq??ïp#="?ïØH
Û¦.?u,œ[aðÌ?sÛúq0¨ï?u,œ[aðÌ?ïȖŸò¬¹?É%}Ó?{´°¸'|?É%}Ó?ïæz3ˆÿª?]ܤ"5`?i…̬š>?]ܤ"5`AGN4FGL J0308.1-2852¿Ðú	Ä­w%ÀMðX>…vÍÀ;`Á¥À<ĦÚ'Q@À$¢ö@_ƒôç?É秄ô¤?´ßª_‡?èC ´@ZÖ¼å¤?ïãq¿_üÀ¿ã0
¿0W¿Øò@#Ü~¿æH¿AHõ'¿Ö
HÞI"¿ïÿ·Û¤%AGNbcu3FGL J0308.4-28522MASS J03081686-2851054?ïþÙ_m=?ooG½î?"j*š1F?ooG½î?ïöC_?T0_('H?Sçù‰{aÉ?T0_('H?ïñÊHÊ/u?VqL/mÕÀ?\knòQų?VqL/mÕÀ?ïý"Réª?óÛå}Ź?3ÝiVñ¤?óÛå}Ź?ïÿ(þb,V?&
_×Ï?à;8IP?&
_×Ï?ïÙp¨ÎY¯?€£)ƒ8²?sG«–Ãd½?€£)ƒ8²?ïò—7зú?f˜¢z*¥?Zя×ß\•?f˜¢z*¥?ïø¬ Ì,®??8—Ó¯ÈG?MM}¤›n·??8—Ó¯ÈGAGN4FGL J0308.4+0407?Þ[í!èiÀF@ûüe@ÌÀ9r×;»—ñÀ<K]Ìcñ@7žÐP?þ"°hè÷¦?²rÐWîï?³»ÀNÓç@Ôþ¢1î@
(Kù}°¿ïkL"=?ïôµ^œ£¿à}Ôvå9«¿ÛÊ÷_tp¿ã¸ÅÿS1Ö¿ÝI‡Þ[?—AGNrdg3FGL J0308.6+0408NGC 1218?ïÿ!VÍþ6?±YW)7'?Õ#]Z?±YW)7'?ïöæ!˜½7?Rð)m?R3¼nP'´?Rð)m?ïó‹y+¡*?Uª©óÂ!©?Xéð;Ø?Uª©óÂ!©?ïø1A7û?7J¾y«;?O:û:"†?7J¾y«;?ïþ–›.çl?4;?QÇv?&–Nwú˜?4;?QÇv?ïÕÎÞ[&?€—;	Z5š?up˜›Ñ-?€—;	Z5š?ïåÄ}î?u½~º­?j€<	 Y©?u½~º­?ïêO½ÖB?Yçã÷+?e°p0KŤ?Yçã÷+AGN4FGL J0309.0+1029?ìwôЙWwÀCÛ×Ûô‡ýÀ8ÜG©â¼ùÀ;¬éïóB'@e'æèW@Îy$¯ò?©çØýî¾ö?½Zç,IŠ
@´'\e[¤@ÕH©0տ؏ØÛMîö¿ÜUÝað_ú¿äEÂÖ[¿ç(àwúc¿çH©©µ¿æE»ãAGNfsrq3FGL J0309.0+1029PKS 0306+102?ïþY)ðqö?€Aƒ€ò?*m^kÄ{?€Aƒ€ò?ïõÛÁÝ/›?V,Z_ºe?TH{Ò-é®?V,Z_ºe?ïàr¾Ç7?sŸ?'^Ž`?oøýàq—?sŸ?'^Ž`?ïÿ¬bk|r>õ½Ÿø¨Lú?ç`PŽJf>õ½Ÿø¨Lú?ïþ¤Z_>v?"ðm`N
r?%ºVtç†?"ðm`N
r?ï؊ë"o¹?v˜ÏÁ/Ë?sºŠiHÑ?v˜ÏÁ/Ë?ïä`´˜
?t¶aäìH?kŸKq"Ýä?t¶aäìH?ïÿ@k;H'?,óޗyà?òœS#?,óޗyàAGN4FGL J0309.4-4000?Û£$åÈÐÀM`_ö"FÀ;[­÷õoƒÀ<ÛÑ_ÄÖ@ ¤{jÚin?ûæ ÆI%
?ËÁ>â=ø?¼(ÝÄÁ»w?óܨ##ñ@ïkY?aj¿ï€x–Ó?ïý Ê]¿ÛD!=<v¿Øtâ*,#t¿åjÛuÜûï?³¦G":AGNbcuPKS 0307-402?ïÿ"ÕE¨?bZ×Xÿ?
ˆ|"¡÷?bZ×Xÿ?ïôÁQ³?Í?YÍS¯üf?V}\¯}æq?YÍS¯üf?ïïsžïU?h*^*´/Ü?`àŒŽk'£?h*^*´/Ü?ï÷ŠÁm%Ñ?9<!‹?Pê}g¬Ýÿ?9<!‹?ïÿ-2EÖ?qàbïW?Y¸)òµy?qàbïW?ïÑp;…ö?qOÆ5\Å?wGâI»$Ï?qOÆ5\Å?ïôtÉ.?hdß(s)?Wñññà³?hdß(s)?ïÜi"]ˆ?ck«Tlá?qË5ÅÍÑ?ck«TláAGN4FGL J0309.7-0745?îm&|ŸÀIükßL+RÀ:`ۋ¬q
À<b//˜t@Çñ²µI?ýï¥Å!á?ċ–€_Œ?·›ùñ9!?ñÀ£"î^î@Oá>Ê?îÂWþė¿ãW²8ÌÐ(¿ßT|Yó¿Ç˜iwÿk¿ë˜š`höd¿ U8»]dAGNbll3FGL J0309.5-0749NVSS J030943-074427?ïöÓƒ‡¬?H½'>c ?RYÚâó(y?H½'>c ?ïõíË}Ÿò?S<ÈK¦R?T$i~Œí?S<ÈK¦R?ï•þUA6<?‰àËN á‡?Š€j¡ôú?‰àËN á‡?ïç­ýeH?P¼ÿœ¥4$?hR@HY?P¼ÿœ¥4$?ïéª=M5?`ڹ퀰?fçU»Ó"+?`ڹ퀰?ïՅSD(W?v4Ór›c?u=VW¼ˆ¿?v4Ór›c?ïœGƓ"?‹ ŒêÚ?ˆü.[7‰?‹ ŒêÚ?ïµ<ôcOí?pÅðfdJô?'°ÂÚuvä?pÅðfdJôAGN4FGL J0309.9-6058¿³ÞaÀ¿lJÀHxj¹¦À8c9‰Ž‰›À;á"0ÉÌg@ýØ@N°œë]²?ŸŠz¨ùÅ?¹+
÷fÿ@‡¹E @¥K#É3¿¬Õ²_ÊQ.¿ãP;å‰\¿ç1tØÂú¿çÖÆz£¿é¹…\˲ñ¿ïïÉQIÉAGNfsrq3FGL J0309.9-6057PKS 0308-611?ïù'_7ÀX?C(/èÍ?Iö"®ë?C(/èÍ?ïö–ÛàLB?TêWUá
Ø?RÒHî\í?TêWUá
Ø?ïÎÕ1—«?|k=õ?x•g'Ñ҅?|k=õ?ïÿªVË?·ïfm0?J¸ÿÉ ?·ïfm0?ïú¦«65W?Eä­Ae?EeR½L©?Eä­Ae?ï×æ#"‹–?xNw>ËKÔ?tîPW<Ç?xNw>ËKÔ?ïÐÝÊd×_?€¸pW'š?w'ÎD<Œ?€¸pW'š?ïüÅ5SÉ×?2`Әƒ›?9ÖTs8þ?2`Әƒ›AGN4FGL J0310.6-5017?îæÜ@ïD­ÀKmÖ¾¾QÀ:*Vˆ¢ÑQÀ<a€OE¸q@ yޓô"?üs$ºÊl?·•`ÏΉæ?©A|÷øI¨?òª—ƒ>äA@%"z£Š3¿à=¢wŽ­?î½:¾AÓuNÌí¨¿â©?ÿÊP¿¬yšÜËٙ¿çÝúºpªAGNbll3FGL J0310.4-50151RXS J031036.0-501615?ïÿ52øáå?¾x
Š|È?Y Ìt!ý?¾x
Š|È?ïøC=õâx?NÓ"§	?Nó‡÷‰?NÓ"§	?ïòìST?a;œ©àŒ?Z'YëÃÜ?a;œ©àŒ?ïþñ×7"Æ?þÃÌ™? ⌬œðŠ?þÃÌ™?ïþ§É£?î÷õౚ?&%Œ£@åÊ?î÷õౚ?ï×Ñø}!5?€Ò©pRS¯?t°AYo?€Ò©pRS¯?ïòTxIµ"?hÝÃ4ˆ à?[W8[«í?hÝÃ4ˆ à?ïýà%D24?'ñ—,?Í?0þÔ©wçí?'ñ—,?ÍAGN4FGL J0310.8-1041¿¿ LєݝÀJ¬7'MLºÀ:þˆ†KÞüÀ<‡]°µ?@ 8ä¥Üs?ÿë¯æâøˆ?Ç-fe§?ž¯×žŒón?؆|¥@¶…8?í¤.}ÁÌ¿¿é2þ'W¿ÅÞo¡ùd…¿è¯Þ|¸¿ÒÔó"õH¿Â.åE¿|ØAGNbcuPMN J0310-1037?ïò¬Ä)÷1?™?¹râø?Z¦w¦'>ô?™?¹râø?ï÷3€`°?TqøˆÄâ?Q˜ÿ!ª?TqøˆÄâ?ïôÝb¤Ãw?Tu˜Ý®?VE:ɶâ?Tu˜Ý®?ïþäñ[Í?¾}"®_é?/¡±²_œj?¾}"®_é?ïþuGðk?!Yg)o?(®?¢´@ù?!Yg)o?ïÝ/ߟ@?rçmÉ 2?qrè/ÛÕ?rçmÉ 2?ïöjÎçˆ?c²\mŠ?S*aø€•?c²\mŠ?ïùl'qÔ{?@ûgéÃ?JM¶çGC?@ûgéÃAGN4FGL J0310.9-3458¿åþVèoÀM¤N¤¨ÁUÀ;cârPÀ<æTe²â@@D[GNs+?ýÆ,Ÿ›;Z?Õ:ý Ë?ÀáŸlÂK?é9¯ž¾œˆ?ù-‰Ó¨ß?ïüà[
‡¿â˜¹Z)A¿â‹Y?aiÒ¿Òɧ~^«¿ëÒ/]•?Ջ÷-âAGNbcuGALEXASC J031057.27-350033.4?ïüC‡êº?2ÓÎi=R1?=ãÁæ[I?2ÓÎi=R1?ïïNEÍ–?gëÔ¦=G…?`±¹÷ä!Û?gëÔ¦=G…?ï­'%B@?"Í©Ùê*?"¼[oÐ8
?"Í©Ùê*?ïçƕÑ
#?MéÍ"Fc?h9j@Ðԓ?MéÍ"Fc?ïú§­ƒ†?B?¯
)«?E½a^
9?B?¯
)«?ï¸-rÌG¹?'
údk¬¥?ô£T%?®?'
údk¬¥?ï­ˆ;^Œ?†¤Ÿ°jI?"¾žVhå?†¤Ÿ°jI?ï_%KáL?x§!»ë>Ú?‹è6›Ù¡?x§!»ë>ÚAGN4FGL J0310.9+3815?ïÂÿ•»­ZÀ0ëã}é9ëÀ:
ZÊPñŠÀ<:"^žñÈ@0z·\Ç@qg#$È6?¿íQ҅že?¹Ç}W™™ï?øÒÅjüZ@äl$ko:?ïà«ÁºJ¿ç4éKˆ"¿ã â-‡!È¿á³/'N¤S¿ío
D& ~¿ï×ó;Ì^éAGNfsrq3FGL J0310.8+3814B3 0307+380?ïúì{,¶?>–",Ã?G¼N̑±/?>–",Ã?ïó‡K¹;ö?YyĦ³i—?XñhVÄ?YyĦ³i—?ïÄ#&[ð}?Ì£-nÒ?}îl䕥s?Ì£-nÒ?ïÃÛOO&6?bß%éÃX}?~Xkª´¦?bß%éÃX}?ïê®>ŸÖ?bmÚ:Öæ
?e€Qÿ9!-?bmÚ:Öæ
?ïÎêÃÐX?z±à^ ò?xŠûœ?z±à^ ò?ï›Ç;	ã¦?ì>hV¼¶?‰16§Þ‹?ì>hV¼¶?ï.¹%ûè?ƒ=ÿ¦$'¹?º(ÜøPû?ƒ=ÿ¦$'¹AGN4FGL J0311.2+6856¿ïË1½Dø
@"͒·þ¯À:¿ޱџÀ<2$fÖ@ ¯ø
é(?û‰Uê`o?ÒEÇ_zŽç?ѝbœ,p÷?û-%g˜•Ž@ æõ—ò%¿ÉÞºu‡@§?ë­ÃAޜ®¿âò¡r«ï¿Ùˆ›dÊÚÚ¿æ$ü=s¿Þ"˜±<MŽAGNbcuNVSS J031111+685610?ïûK±¤?;Õ$ÿ*';?BÑ<°Ç6?;Õ$ÿ*';?ïæ$ê›í?i›ªó¢È?iÛt
ZÎ?i›ªó¢È?ïÛ!ò¡¦6?qkó5M\?roÁºÈÝ?qkó5M\?ïÌrÎB?\#¨M©è…?yÆýÀ?\#¨M©è…?ïøÕ|§N?IQoåeR?Lª
ìc!?IQoåeR?ïx¨'?"b/"–ÿ?êýï—m"?"b/"–ÿ?ïŽ ìrÒ?ó Àâ*N?Œwúz"wš?ó Àâ*N?ï<zNО?†¬"MM†?˜lP²¶PS?†¬"MM†AGN4FGL J0311.5-4402¿×{ŒSòÊÀLž¡3ßÀ;e'Ýãu†À<ãñx7@YvT3ˆ@pµ'-lJ?Âϼ<0Þ¿©in"?åkÛ@#œ@,¶ùPäI?ëËw͖÷(?í+¡~•\H¿ãÝløPß¿ïÿ ÿ¿h`?ïý''N#z¿à¶Y"±ðAGNbcuGALEXASC J031103.24-440227.8?ïÿž—k}8?¤Èâã<H?Z&°	Ò?¤Èâã<H?ï÷Áa×ü?QªÄˆ\dÃ?P};ñÆ÷ä?QªÄˆ\dÃ?ïÈ}ô2Óx?ƒR#6™?{ÁõŸÝ?ƒR#6™?ïÿèÏH
q>çg¡–¦ÛÕ>ç0©'EâD>çg¡–¦ÛÕ?ïþqH}Ù[?.á[³g?(ët]Ja?.á[³g?ï×;A¹L¬?€hj;˜'?tb_Š5ú?€hj;˜'?ï¸S2yqR?‰¤ÿ2¸‡?ë3iâ»W?‰¤ÿ2¸‡?ïÿP˜î}?cõ:	‡	?ìý4…få?cõ:	‡	AGN4FGL J0311.6+4134¿õ.&LúÀ,ô{gkÀ;z/—@À< !úü‹@!mˆô…Î?úO}¶åû?ÙFf@Ѭ[?Õ,ÅÛÁÝ0?ùoz^Ù@g"#ìÞ¿Ñ5®ÃLpq¿çæf0¶1¿ìNÚX¦ŠC?º#Rë__¿èe;ÞÓ_Ž¿µ 8š%Z­AGNbcuB3 0308+413?ïû¸Yðƒ®?;'çÅà?A—ºá?;'çÅà?ïô7–*Š~?V›ºŸ¨?WÓn#r?V›ºŸ¨?ïÎ:LÐ?q"³í¦‹Ã?xâñ™6O¤?q"³í¦‹Ã?ï÷ë
?;uTò¹?P*Hz«É?;uTò¹?ïõJi}ž?]ÒÝ=ÎcÆ?Uk-‰ÉÂ?]ÒÝ=ÎcÆ?ïÎßY—K?€ÈSùùÁþ?xò?öŠ•?€ÈSùùÁþ?ï¤OÑã?‡Ý<§=U¨?†ì;F	÷?‡Ý<§=U¨?ïÓô®_›¾?m
Úuå.ø?v¨¼Ddï?m
Úuå.øAGN4FGL J0312.4-3221?הª˜*¿ØÀM‹ºÜ	€²À;ylÛM™À<÷#a	/@Þóú?üã¥Áƍ?ÛæŸê$Ì?Ñä"''?úNãx	üÙ@ía½ª?ï±ÊÛ[¿Ñü×V"ŠŒ¿å¡@Aº¿Ì!8	ã¿è)Âbæ¿ðAGNbcuNVSS J031234-322315?ïûFâ†â?5¨ÉAí«?Bçé6N–r?5¨ÉAí«?ïòýþ?'ï?\ø'¼i??Zh<ñÍ?\ø'¼i??ïÇÀÔÁ?w¤­{Ó$ö?|•èÑ7…?w¤­{Ó$ö?ïíü…ª¬ð?F´(qÌ+?bzYPa?F´(qÌ+?ïû&‹sÕÔ??ë=€€D‰?CeÑÙÌ(6??ë=€€D‰?ïÏ"‰å?'/Ž]-\?xnºñI®?'/Ž]-\?ï¤x[±?…n۔‹žÌ?†üxÞyw¯?…n۔‹žÌ?ïÁ™Ð¡½?nÁSfžÂ?3Ðpa7?nÁSfžÂAGN4FGL J0312.5-2221?Ð?	)8LfÀLÛƒjƒ,À:8†-¬
µÀ<bãv\}¯@ N™@-m?ú®4Ʊ)Ù?Àtv‰õÛ?ÅF×)òíž@I¢ÿsé@Üwý½…‡?ïÿì´É È¿Ýq ~¥¢f¿°¸'Ï&ï-¿×⛠}.¿ÜXJy¡¿ìy&\‹RAGNbll3FGL J0312.7-2222NVSS J031235-222118?ïû"ùéÝÌ?9¹(—§]ì?A°[Ô'?9¹(—§]ì?ï󺽴3¬?Vê Á%ڜ?XŠ"Gá·´?Vê Á%ڜ?ïÝTK~%?tò<ªI¤î?qUÚ=}Ø×?tò<ªI¤î?ïÞÖÊ3?RzEæÉ+?p"šãçâ¥?RzEæÉ+?ïô}p̤g?RQÂ&…ë?WÁlâx?RQÂ&…ë?ïÓl±t"?w´$AÎ5"?vI¸
ؚ³?w´$AÎ5"?ï¥Á"Ú?‡z",¾è?†›>	zþ?‡z",¾è?獵P³Ä
?rZ¸z0Ðß?†V+Ì/Å ?rZ¸z0ÐßAGN4FGL J0312.8+0134¿ët³¥Ö¶'ÀF½ke©¨À9ƺNEqÀ<(ó"Çz}@‹‹«sÄ@-òˆH?ºùµkŒ&?¶U¶ë¹÷Þ?ù˚¥—Õ@»I)"£æ?ï͐â:ó¿Ñ!DÚ$¤¿åMú>ŸøÙ¿ããe€À¿äéëÁ"š¿ðAGNfsrq3FGL J0312.7+0133PKS 0310+013?ïþ|ϫƺ?*®h??(3Ávú?*®h??ïöL&c÷?VŠ¨Fyñ¼?Sg³"«Áå?VŠ¨Fyñ¼?ïë`@‡"™?gmæ}™ÿ?dŸ¿°Ôþ…?gmæ}™ÿ?ïþ#B5•Ê?•Ý±¾.9?-ËÛ
ž«.?•Ý±¾.9?ïþˆ§êüI?m²§@Š"?'u}£Ü	?m²§@Š"?ïÙŽ%?~HÃÂOÙÒ?spü>lÞ¹?~HÃÂOÙÒ?ïØÊâÅe-?{—³,?sšŽŒÏI'?{—³,?ïü!Ù;›?/vÙ)O?>ñ7T·J?/vÙ)OAGN4FGL J0312.9+3614¿¥'Ù•†Z:À2i¶°_¯À:ieõ'_À<?
 ë2@ žôÄ7§â?ýYÞ7X\?¸Ã…¦G§ß?«I­âÀ˜Ñ?óÚE[Sã­@±(Íÿ|Í¿ïýgß?ïãϝ·‹r¿ÈqMàˆ–g¿Û±dÜ£"¿äeÜÓ«
¿ÃÏéŒÌAGNbll3FGL J0312.7+3613V Zw 326?ï÷w¾±Õ?‡‡Ð'üòz?Q'åf6l?‡‡Ð'üòz?ïò–嬏?aA©ÌÏG?ZÒ4>mÈ^?aA©ÌÏG?ïâ tÐȖ?uýnÔi¼A?mߋYr?uýnÔi¼A?ïÑM¤<z?`›Û"™F?wvÙ¥3\?`›Û"™F?ïöâOj÷E?HûõÙª‡?R;aHNK?HûõÙª‡?ïеe/¸2?whr{6Èå?w¥Mj3ªó?whr{6Èå?ï芕<40?uwwø?gukDï?uwwø?ïi+¬?Ö/Ê:?'ߎ±ÙÔ?Ö/Ê:AGN4FGL J0312.9+4119?՝qEùšœÀ,7A¿½ð'À:7"¶
m§À;
ñû@§Ï"þ)f@+¹!]¹?»O'ÿƒð¿¿W4ð!»'@f"f\Uk@	¼óíx¿ØÔDRÈû¿Ëcòl¿Áj¢
Vp$¿é~0O‹Y¿ÅV1ûOÂ
¿ðAGNrdgB3 0309+411B?ïø2;fˆu?UÈJÒL@³?O7'Ln;?UÈJÒL@³?ïñz£'Ê?[6)y¶'?]ÑRJý?[6)y¶'?î¼ûú%º?›xbŽ›?¤>À<îa?›xbŽ›?ïúmáHɌ?@4Ñ-{Ѽ?FH{î¡í?@4Ñ-{Ѽ?ïÚmG3ÎÂ?}À²¦›?rÉ\l÷Öå?}À²¦›?ï±BNq7?ˆWv¡v`?ƒ¯ly+ä*?ˆWv¡v`?îj›\g_
?œÐéÀb+$?©VJ<Ä_?œÐéÀb+$?ïƒNí+´?¥Óü¦`%?,~Evî?¥Óü¦`%AGN4FGL J0313.0+0229¿Àgì£VܱÀFhfýe
À:×+•°À<1œñ<îž@•<F,_/?þŸ°i¿·;?ÜØÄ|Ç%ï?Þùà@ÇñF?ûë ªšrÝ@áão{ë?Ûh $ã1¿ì;P8&¸¿ÝdgE‹%¿èIŽ;Tj¿ïÿÌÔY‰¿ïÿþÐñAGNbcuTXS 0310+022?ïú¿—b»??G|ÖÂÓ?E¡Û±BÀ?G|ÖÂÓ?ïõQYu"}?V'VK,z?U]Lä@¦?V'VK,z?î¬×dˆô8?—¿CýNØ?¥2‰¹(Šv?—¿CýNØ?ïé¯Â-•?Mïz¯¤÷¼?fP=û¦8•?Mïz¯¤÷¼?ï÷†ä'˜n?QF¤gp'?Pò7E´k?QF¤gp'?ïÒǹF?ÃÌuÒ?vœ#n
‰‰?ÃÌuÒ?îˆ&î½s¥?š¿$ä(¨?§}'¼z²?š¿$ä(¨?ï¹K?qA"pz.w?¹>*€,Æ?qA"pz.wAGN4FGL J0314.3+0620¿Êì+"4¥ÀDñLìAÝÀ:\¶wòÀ<:Š:N@ Ώՠ…ò?ün 9[ka?Ɩœúw*?½[$À?ôdõgö‰_?÷Տ;qÆ¿±§Ð(Q¿ê^ǀ݋¿Ø oA{P¿ÉWX×\»¿äíÑÅZ¿Õê€Ý
1²AGNbllNVSS J031423+061955?ïüס3ŽD?-ÝiÀ=?9BøhSð?-ÝiÀ=?ïêÐû'?fíËQLû¾?eâ/én'?fíËQLû¾?ï†ä®?[QnkpKú?`jyB!'Á?[QnkpKú?ï¨é'Ä?h"ÿȘ?…Å»-	šÖ?h"ÿȘ?ïû¯a4«â?;‰FÆÔr?AB|;>"?;‰FÆÔr?ï°€v\ÿ?†ôï"O?ƒü_×jm?†ôï"O?ïêÛÑ«?pÙ\ÄDÓ?e$.™¬ ?pÙ\ÄDÓ?îOw†–©ò?"¾½6àE?«‡™)Õ?"¾½6àEAGN4FGL J0314.3-5103?í=÷ßõôcÀJü©iuÍÀ9¨²ã»-À<XKƒÂ@úñw§Š@u_þmY?°S	<i½´?¤-?SR'?õ²`Š"Rà@ˆýµLþ`?ïè'á´,¿â±Ÿµ<O¿âtô3C#k¿Ý¸ãÁ…ñÇ¿âÖÑ"qïÜ¿Þû:]ôÒÐAGNbll3FGL J0314.3-5103PMN J0314-5104?ïþÈÂüêL?"9Qy»±?#sÎëæ©ï?"9Qy»±?ïözâŽ÷?Un$¡Ñ?S
:xšC)?Un$¡Ñ?ïø¬!$~?\¬ñ÷=?MOzÇvÛõ?\¬ñ÷=?ïûöÄJ¥É?+ö͈Ëï?@$ïË&ƒƒ?+ö͈Ëï?ïþi»ÁÖ?SW®‹?)dG¢µÝ×?SW®‹?ïÚÝY
Ð?tÛ´÷`?r'ScM,?tÛ´÷`?ïù¿£¢?\G®¼Æ^?K¹Sjà¤?\G®¼Æ^?ï÷ÉSÃu?@3ûm'?PmXëúõŠ?@3ûm'AGN4FGL J0314.6-6549?ï
?§	ï˜ÀF¯mÚÎîÀ:ʘòª¬çÀ<¡öé	:@1ª‰€ò¯@')Àê?¾"ÛÍÐf¿—àõ@?ƒ?ÕÇ,#õR¨?üêõçÎ/ù?í™ö`ÄæÏ¿æÞÕþ¤¶-¿æ·é{Y<²¿åK¢•ÁÅ¿Úaf'–¿ïþÊ-ëÌAGNfsrqPKS 0313-660?ïûê)²‰ˆ?3%G_¢¹‰?@WYÜmT·?3%G_¢¹‰?ïò).¼DÙ?]{{s®@w?[­¢i9¾?]{{s®@w?ïß&Ÿ¸?j±ÿx
a?psø€ßÐ?j±ÿx
a?ïôUHBE??É~þÞUµ?WUoüòÄU??É~þÞUµ?ïùÎëé{?DäÛNm®@?K"Å7uM?DäÛNm®@?ïÌlê†h‡?q3‰CZ?yɊÛLq?q3‰CZ?ïÏa~Âu'?{ó›R?xO@ Õ0G?{ó›R?ï²°~.üd?s]ŠŒm܆?ƒSàz<ê?s]ŠŒm܆AGN4FGL J0315.4-2643?èCÖD"wWÀMYÝÁç–À;M¶Šk(À<¼½qåöi@!
K^"E?ú¢Ë;Óå?Él'Ê !É?Ǎè5ˆøâ?þD*Lä'@žq-êžð¿ïû—?ø¡¿ÝùV-3>ò?ïùÄýuŒ¿áaÏ}×Z¿àž+ϑ£+¿ãåªê#õ©AGNbcuNVSS J031527-264400?ïýdË+?,;'Ø
?7\ÚÕ{û¥?,;'Ø
?ïôUž±Ë-?U€/Ø»8•?WTÂ÷T"?U€/Ø»8•?ï䛈åŸà?e;²¿¢›5?kdvò"¨*?e;²¿¢›5?ïäÈ4±?Vr(o$?k7ðú®þJ?Vr(o$?ïùQ©Q-Ö?E2Ú1âÁ?J¹Z$×ñ?E2Ú1âÁ?ïÑðöLÍä?€í«~óIê?w"÷%±Ú?€í«~óIê?ïÄ®§Œ6?~ßÀ"¾åß?}¨¬<w•9?~ßÀ"¾åß?ï¯õ%'ú?y=½ò´©?"¶¶{£?y=½ò´©AGN4FGL J0315.5+4231?»"Ǖ«MvÀ)¨Ût´À;lŠŸ*ÓÀ<—!Áçã@!rg‹T‡l?ôû…—"¤?ÜýŸ—Šv?Ý×(›T¯°?ø›ÌyÁ@A:¤Ék¿à>ÀÕó'¿å*øf®ŠÂ¿ê­Ù!nå'?µuc.xŽ\¿ãâÌ'ª¿äµðè5AGNbcuNVSS J031527+423249?ïý"ýV
+?-ÉòÚU?3`(I71?-ÉòÚU?ïô#"jìÄ?VƒÜ˜±X?W¸×78?VƒÜ˜±X?ïÈKtãñ?uïn|{Kß?{ÚBkM?uïn|{Kß?ïùçx'a¡?4[jßoÛ?Hb X«?4[jßoÛ?ïüMië?>ȖˆøI™?;\¯ýÛ?>ȖˆøI™?ïÇjI
ÔÄ?…ìŸÄ䝏?|JÛ[ˆúT?…ìŸÄ䝏?ï±x…DDu?†Ù¤*ÿùn?ƒ¡Þ¹í¢´?†Ù¤*ÿùn?ïí|¨‹ê?XHW|äÁ?b냖¬æ?XHW|äÁAGN4FGL J0315.9-1033?æOÓï£3ÀJŒCoÁYÀ9‰ÞNÕP)À<8€eëí$@#Pn'i§@tpë$¦¨?± $"I+?µÈNŸ¥m@uûdÌ'@CîÅ&?°È`VìÕ¿á9äþú2¿è𯮯¿äŒ <Àü¿é/–Ð<¿ïñneZÎAGNfsrq3FGL J0315.5-1026PKS 0313-107?ïþAÚ	Ò?>x:îÁ?+âbéN:?>x:îÁ?ï÷R%"	¦?R‡ÈçÇ?Q[¶)à2·?R‡ÈçÇ?ïí,è…(ã?P¤BòpY?bÓywDð?P¤BòpY?ïþօïSñ?››¾2ö_?"—žÓgÑ{?››¾2ö_?ïþ[êÙʄ? ·[|´2h?*AOîlú? ·[|´2h?ïÛø_ˆâÎ?s¯d;Ó½š?rÐ$á,ö?s¯d;Ó½š?ïâœÙPO	?oþܘ℃?mc&s7×F?oþܘ℃?ïý6Åõÿ1?)&å#v?6IÑwË9Ò?)&å#vAGN4FGL J0316.0-5626?ŸeC¦äÀI€Ç`|À;"¶Ò"mÀ=½‹ç)@ .ð%ä?õe¯ò¡r¬?ä=n q¥	?ä:ß%"å@÷üü?@•Æ1}%›¿â"ií£ù¿áß
váí¿ã‰Â@׶‹¿Êùá'çQ¿â©9êÝY¿ïÿÿ&¦³AGNbcu1RXS J031613.4-562545?ïûÑä}‡Y?9ˆ> (žŸ?@¸n‡Ç~4?9ˆ> (žŸ?ïõ~^à?Tg=4i˜8?UÉZs'?Tg=4i˜8?ï -ž™6?ƒ%žÝÇå?‡ôŽš¨†s?ƒ%žÝÇå?ïöÓKl?<ٓaJV?RYiˆÕÔ?<ٓaJV?ïû@sk:>?DߙxBÇG?Bþ2$éí?DߙxBÇG?ïÕ
®¶¯?v¿3»P?upy9Ò´˜?v¿3»P?ï¹î(Q?†yi%òþœ?"z5>½ã?†yi%òþœ?ïæÄ"Ÿ"?`œ±±ôå?i;ñ²Z;Ó?`œ±±ôåAGN4FGL J0316.2-6437?×ìéâԘÀG|"µÜÆÀ9êHX^eçÀ<3Ð&ô`@fyɹå?ùpÃLŠÆ?·N[ؘÝÝ?½û&Qxm¥@	›ü"$íö@ƒýLŒx¿ÒLŽ£ò8¿£‰9¥H­¿®·}bßÑÀ¿ÒŠ4¸Œ¤¿áqÊi¿×ÙFWÓ%¬AGNbll3FGL J0316.2-6436SUMSS J031614-643732?ïúLh¶D?CjÊ{‹¼?FÏÑgö?CjÊ{‹¼?ïóññÁÆ+?Wê'_Žå?Xܨ¹§?Wê'_Žå?ïéwCid?k5ôC9ã?fˆ¼Õ›kî?k5ôC9ã?ïæÞ["O?ML
ÖG–ã?ià!©û?ML
ÖG–ã?ïçð[6 g?gr援?h¤¼!(Ñ?gr援?ïÔX&,©?vã|F¹?uÓ÷ë‰Ó_?vã|F¹?ï­¦ŽAF?‰•IË•Ú?"–\v™&'?‰•IË•Ú?慨Âíc?q‰pÅ?…ÐOy•M?q‰pÅAGN4FGL J0316.2+0905¿è¤vfPRÀCɤi×4/À8¹g«
fÀ;«ÇQbÉ@®Ô²?ýЕÊ@r?©`¢G'Ý?®õ|æ§â@¸G¢'v@9Äè§É³?ïöæç*F%¿ÙÐwœn¶¿Ý©·ôÎs–¿ÚCyÒSõK¿àðíޕL-¿àí¯e³¹AGNbll3FGL J0316.1+0904GB6 J0316+0904?ïþç·½N³?ö[Á8Æ?!"… êL	?ö[Á8Æ?ïõËV³ž†?S
º«y?TiR©A³?S
º«y?ïænñAë?uÌiáTH?i'ï}Å?uÌiáTH?ïöQâ1A?A2}g¨ë?S\;qÈ}³?A2}g¨ë?ïýâZÉ?0éÑá"2€?7(ðÛFî?0éÑá"2€?ïÜ5õÒ¡ð?tmó?qåù"d?tmó?ïÕã¶.Ù?åì¨ê*e?ux›ù—o?åì¨ê*e?ïî™IMâó?Q'aÎ?af¶œ?Q'aÎAGN4FGL J0316.2-2608?îYώ6þ´ÀLݍ%íÐSÀ9ÇøåY‹À<6@<H†@…[f=r?ücZ'ó+?µ\ÿ	Šî?¹s 
Ìã@Ì|Dôü—@PhÖ-H¹?Úöóý=Wú?Ïk>¬¿áŒY	†'¿Ð娶m¿äÕ\Rç-¡¿Ù›2Ál"AGNbll3FGL J0316.1-2611RBS 0405?ïûŨìô?5Á£·?–?@é\Ê$¥
?5Á£·?–?ïï•1³‰ã?`›0|-zÈ?`jÎaĘ?`›0|-zÈ?ïçÔCéd?l(X¶ÂK?h+èª8¤=?l(X¶ÂK?￀ԯLè?ckÛÅ1ÿ?€ÊÆÆL"?ckÛÅ1ÿ?ïî÷öWpæ?WÍõòÛP?a	"ñqÄ?WÍõòÛP?￧O17þ?sؘž¤?€,B \|?sؘž¤?ïºÃ")´?"]ùs1š"?O7¾´ñ?"]ùs1š"?狀Í#'?‡9õ×ùtÍ?Ÿk®ò"¨?‡9õ×ùtÍAGN4FGL J0316.8+4120?ê]X,´5tÀ+g0«¼²À:z®Žd•À<	›h¦²‡@"YBI-Æ?ý[8jª˜Å?È=º ¥Q‰?¾ú|2€†@Pÿ}¤§?ç:V[Vh¿íœý
y¿ÙBW}ë=P¿åqÏ ¼£Š¿ØÑN;Í5¨¿Ð¸
ãmx)AGNRDG3FGL J0316.6+4119IC 310?ïÿú›M?sÔÚ>~û?þ{Ý"ZË?sÔÚ>~û?ïö`Õú?Tõ'U•K?S>UÐþ?Tõ'U•K?ïôi'¥¥/?`†p+Ï?W-°¿´a?`†p+Ï?ïü$'°&?+bå~¯??fÜÉÑÍ©?+bå~¯?ïþð'Ç>?±HhD‡j? ý‹Æ]y?±HhD‡j?ïіjåüõ?ƒ¡>VºeY?w4ʪŽ)"?ƒ¡>VºeY?ïñø%ž¨«?kð¿gµ?\´Êíº†?kð¿gµ?ïõŒ*	?I[¦
`t?UÆçÏj]'?I[¦
`tAGN4FGL J0316.9-0625?ïSCu÷¢ÀHÞìAÝ"À;Ÿ†B¤ÀÀ<©ÓåjS@ "DðIÿ}?ü,?ùë	?ÑA ^Y҄?¿¬œU¶•Ô?íÞ½ý&1@aÒ"ø¿äEå½_¿ë5ßàл¿Ñ«±EX¿ÝÒéý	U"¿à»ùu¢CŒ¿×]cß#'AGNbcuPMN J0317-0623?ïÿ"ÿx4‰?ìëM&? EÛ«è?ìëM&?ïöHîSÛ?T-ˆ6¸Sd?SoÔs9T?T-ˆ6¸Sd?ïóË6A'?päC'M?XÞi;‡²h?päC'M?ïü†ë¹nn?#Üvâp¢—?;È¢E
³O?#Üvâp¢—?ïÿ9uäÕú?)¬ªÂÀ½?Ñ@O2.?)¬ªÂÀ½?ï×èjž?­?v‡tšÝï?tʟ1±?v‡tšÝï?ïú´Xë1?X½":,;?G-ØbÌ?X½":,;?ïós.Êã?JêK²Ã?Y£˜2ªº?JêK²ÃAGN4FGL J0317.7-2804¿ïS©Ý€ñyÀLÚ'¿aª?À;ü/çCÀ<Þè	i5N@A`[	ø@þãþA¹ß?Ótá¾ÌY
?§ÂIÇI?Êê›ê¬±¤@pM
ú¿y¿ã-Æèl¿Ý¢}ÃÐ#ï¿çòbo¶Ç¿áhœ|&¿å#ßYw¿ïÿÆߢèMAGNfsrqPKS 0315-282?ïýfœ…öé?Mºl¯úÔ?4ËP½œñ?Mºl¯úÔ?ïöÌõً?PôVø4®?RgLé?PôVø4®?ïáCl;gŠ?{'¯ƒ{v?n¼"•"?{'¯ƒ{v?ïþ`€üÈF?nÇ"Jôñ?)÷îlIð?nÇ"Jôñ?ïÿFr¼FS?4ì"
?$?1¢E¶´?4ì"
?$?ïÙˏú£?t†®ëqü?s|šZ^Æ4?t†®ëqü?ï䫶Q¶+?w'vÛðQ?kTI·è¼Ó?w'vÛðQ?ï÷Ñ¡"î?BñŸ0Ôκ?P\¼w—ïÌ?BñŸ0ÔκAGN4FGL J0317.8-4414¿¥Ò¯6<gÀL´ûß	À;¡óQ›ÔÀ<ïq"§š@!wi¹'G?ýnvÖ 2¥?È0î	ˆiñ¿Ž/¹gP'?Ç?·e‡nI?ý\?r±£?ïø"à4ê¿à L jÓ¿ç3f"‰`¿Í›ÅÃď¿æ¢BŠ"?УßBÆ#AGNbcuPKS 0316-444?ïþ'妰?Þ#"`'æ?&î]âhî¯?Þ#"`'æ?ïõ´#ð?VÔ@Ë(ˆ6?Uؘ0¯n?VÔ@Ë(ˆ6?ïðtehË­?e'Òáʙñ?_53è³?e'Òáʙñ?ïøÑG°Ã­?5LµŸS?LºàF+-?5LµŸS?ïþ»J!ÿ?ÏåWF†¢?$K_Òzµ?ÏåWF†¢?ïÒO¦´?€ÝÔ!ûáa?vØ-
·F%?€ÝÔ!ûáa?ïð‰4>Š?m~=ï¹Â?^í—L×+ó?m~=ï¹Â?ïÞi,òÚÜ?b
W݇X?pËi~S'?b
W݇XAGN4FGL J0318.7+2135?ënZ‡q41À=¢Ž£œQÛÀ9{¤ÆôFÀ<˳È	@ÐõØ´·'?ÿõ±]½Õ?´¨ÜW¯>q?°¥¿AÉÎì?û‹ÐÚè@	T¯ƒeД¿Ùs†Ž$¿Ùv€d¿â_Ïoº¿Ø|10É¿åE!ýÖ¯û¿ß
Ë |âªAGNbll3FGL J0318.7+2134MG3 J031849+2135?ïþ›œ´Î?G½<̂?&O×åè<±?G½<̂?ïõùâÀª?SœÒړ?T;ßÁ|{?SœÒړ?ïöOïpT–?`Ú£Ÿ3æÒ?S` Ò_•0?`Ú£Ÿ3æÒ?ïò†Œ-˜?C&©ÂŠË?Zóó?šÐ?C&©ÂŠË?ïýµ}Oáë?$uzʟ°?2Tþ?$uzʟ°?ïÚéì©r;?tå}×
:?r‹	žèJ›?tå}×
:?ï÷±íë±?[‰M:Ø-}?Pœ%Uöä?[‰M:Ø-}?ïÔ¬3hüÝ?bñˆ9¾h?u©æR`É9?bñˆ9¾hAGN4FGL J0319.4-7045?³jÛ¾r»
ÀDÕa^¿¨øÀ;TÔ«¾_LÀ<㤢â¸@ ÐtcT8<?úW£öíô?ÏûÉ,9?ĺH¦7Û?÷Yn€ç-?ükà£Ä¿ççΰқC?âÞ¨—c^t¿Ô›½ ´ëۿ܌"aFA¿Îº…@q4¿épTü±–æAGNbcuMRSS 054-102986?ïþ8
HÏ
?3¢î¸Z?,+9â}*?3¢î¸Z?ïñƒ—ññ?`RQž:a?\øϝ¬4¼?`RQž:a?ïéé3"›?^|ŠI*z'?fͶµ:?^|ŠI*z'?ïó]˕Ȳ?BFÀ"{?YDh»±k¥?BFÀ"{?ïü†ÄˆcD?4(5©§?;ÉÚeÙ®Ó?4(5©§?ïÄãÀ•m ?"†Mtm‰G?}ŽËöÛ¸?"†Mtm‰G?ïãÊdèŒò?oUg:ƒ€?l5›JMEù?oUg:ƒ€?ïō!ñA?pš)w8ï?}9o.ÙS»?pš)w8ïAGN4FGL J0319.8+4130?ï@ÌÁd8åÀ*" _ñØÀ5Ó²Jj‡À:H¡¸é@oÊ·sÊ'@_&DÉ^?"sÚ Ó}I?°œ}#Â'@'<-ðÔ@ ÷½1ø¿Ç>¢Q#¿ÚáÚ»wåÀ¿â#%¿,P@¿áe°ÿì·¿å`ð
j¿æE~ßÙïËAGNRDG3FGL J0319.8+4130NGC 1275?ïhCPÑn?¢£2¬0¬?'ü7NÌ[?¢£2¬0¬?ï°Cº(
?"V=µ~bÃ?ƒï …À·?"V=µ~bÃ?íæYP1?§å0îJÐþ?·Ï,NJù?§å0îJÐþ?ïñµ©3"V?buÀ*×H?\"­Y¾…?buÀ*×H?î5ÃON+?°L~?%N?¬£Ë›U?°L~?%N?^ÏTx?ºYø³ŸC?¦—Zwˆ?ºYø³ŸC?îËzi?§ÕM$"?®ODfu?§ÕM$"?ïžD6Ül?ƒ`¡ëîy?ˆnòu)­?ƒ`¡ëîyAGN4FGL J0319.8+1845¿ÇV—%öߛÀ?²Ë…¤ðÀ9ârkWfïÀ<
øGv@!xH¥á%Ÿ?ùބ 
Q!?´½cù#ÂÓ?«³4uR't?øšc
»@;˜Í@åù¿ïöÇ¡Р¿–<¶áöL?ïÿÂWþė¿Û¢hu4¿Òܞ¼n/Þ¿Óg/x°kAGNbll3FGL J0319.8+18471E 0317.0+1835?ïÿ]
ªÁ?Ëw£'^?^RdN~;?Ëw£'^?ïöçRŠ?R&ÖuÆjX?R1ZÓ!°î?R&ÖuÆjX?ïôžá¾1»?^â'vΎ?VÂ<*ës?^â'vΎ?ïýí¨ÜÏò?[¶]°´Ö?0'·÷;ž?[¶]°´Ö?ïÿW¡ý?ѹ`?ø?^˜šŠ?ѹ`?ø?ïØo"i\n?tâôÆ)ß;?sÈ6Ràí'?tâôÆ)ß;?ïç>èò?võÜôå"?hÁáqå­?võÜôå"?ïý¦?*Fyš¼Åä?2υã…Ýï?*Fyš¼ÅäAGN4FGL J0319.9-3821¿ìtóËû<ÀLˆ¦ YŸÀ:×ÜhKBôÀ<¤vtÑc5@JëêI_o@šތò?Ã0èU>v?¡"!ý=$?Ú'Òûº÷@	EBҍ?ïç/ï±Ô#¿â'eÀ¤"¿èÙà[DŸ¿é‹¾dª$¿Æ{ò>ÌC¿ïÿÿ" 5•AGNbcuNVSS J031957-381527?ïÿ'˜3
?k+Û4£ô?MZÍ?k+Û4£ô?ïö÷…TŠ"?UpÁºD<?Rõ0o9Ä?UpÁºD<?ïðù
-Ì'?ZŒV`ñô°?^
塨w?ZŒV`ñô°?ïÿ]È'?YIRM?W?FòN¶.?YIRM?W?ïÿ@ËÞK‹?ºo$l?æúϓ?ºo$l?ïÝRà'iŽ?r0ø^㝙?qVÖ7´Á?r0ø^㝙?ïå¿®Åêt?q-6""­?j@Q?"ë·?q-6""­?ïýHý8¿(?-d¬`"2?5¸E†?-d¬`"2AGN4FGL J0320.6+1125?À¢âØý²žÀB¤WÙÜÀ:·ŒR‰9ÐÀ<õ0™%@ Wò ò@… æ"ôï?Âó"`›2¿¥>" šœ?âhâý¹÷@2®Å$⸿Áe¶}ªû—?ì=ÙI²Ñy¿åç-É¿â(<县ⴜ>ån¿ÑXü…÷ü%AGNbcu1RXS J032037.9+112503?ïû¦^E}?<€ƒçäQå?Af…ö:0?<€ƒçäQå?ïñÞç×j5?[Í;<ÑÒ?\B0´ V(?[Í;<ÑÒ?ïáê×ÿ?upÁxK¼O?nog9Ê¥?upÁxK¼O?ïìýMz?IÃFäÄ–?cãÆ:UÌ?IÃFäÄ–?ïóŇçž?V
¦ÖËØ¡?XtïËl‰?V
¦ÖËØ¡?ùӍ?~ç±;Œ?~¾£–T	&?~ç±;Œ?ïÌG
x;?FŽŸâ~P?yÜzäՆ ?FŽŸâ~P?ïpXu•Œ?'ø¸¨)Z?'ýÔñMN?'ø¸¨)ZAGN4FGL J0321.3+0425¿¿š`WÈW·ÀDÿ†ã´oßÀ:§S³ÜÀ</ý ª/@,ÂìÏ º@!_Ìr?Á4ˆó¯¿ª3j¾9?ê‹ÀBzÎÓ@äÉ?ìºåC¼s¿ç±à¸<¿æÏu¹Nk¿á|øCsW¿é&È÷U6"¿Î÷_]ÂíAGNbcuNVSS J032130+042628?ïûCšC?9^7ˆ/¡?BóÍÓšu?9^7ˆ/¡?ïõÚu?R@jô(¨?Uù¬V?R@jô(¨?ïédk-Í?eYŽ^±?f›"áòûj?eYŽ^±?ïö%Uv?7ç¹^€Üu?SµÚüë?7ç¹^€Üu?ïòåÍúŸC?V4Êjýcë?Z4d
Áz?V4Êjýcë?ïÑã'h`?€a»x
ó&?wuŠˆ_Û?€a»x
ó&?ïΪ;8¡m?~nÊ@?xªâp½Í??~nÊ@?ï¶{Ô¯Ç?ot|'F?'a
ÊôÜg?ot|'FAGN4FGL J0321.3-1612¿ãë–Ñ_¥úÀJÕf@¦¹=À;p%FáeáÀ<Ä#G,å;@/ëîÑ?ý橝ÛÙ?ܪ'zÁg>?ÔֆŸkë‹?ýÕ½6VÔ"?úBöt»ê?ëw¥ˆ»%?ï°iŠU_¿áj¿ÜÌú61ë¿ä,HÐ(¿ïù"O¶!AGNbllPMN J0321-1612?ïöÙïÜ-?K)+½7?SôK¬ÔÇ\?K)+½7?ï²Á]ØÎ8?'ZÍÖâû7?ƒO¨"üþ?'ZÍÖâû7?ï­ÿnN?yÈËrœ
%?"€$bê?yÈËrœ
%?ïVÙìx—I?{á}'Ó?•$Âj
Þè?{á}'Ó?ïñÕhãÕc?T¾ßRž?\U.gé`?T¾ßRž?î¡8()X®?± ª8óóu?¥ì}~F\$?± ª8óóu?ï{ÿ~6"?‹×OŒÏ?€4T'?‹×OŒÏ?ìÊŠx®+?¦#oL´§?¹¯¬:Ž¥?¦#oL´§AGN4FGL J0322.0+2335?ÒöÄK¸©ïÀ;˜§'h˜À8ßaúÆÛÀ;М·[K€@^æÀ=ó?ÿƒëaãIç?§uëƒ`?‹~Ö¨KkÂ?ãYA¥Ã@øù²%?ïô5â:\¿àñ¦ é4¿âúúÁ»¿Û'ýûÉ¿àÃhjL¤ô¿Ùº å¾5ZAGNbll3FGL J0322.0+2335MG3 J032201+2336?ïþ}"?!§öï›K?/7Ú¡T?!§öï›K?ïöIžQ?Wi'ϖI?Sÿlçä2?Wi'ϖI?ïì=.Îcj?rÑt3$
ô?cÂÑ`‰?rÑt3$
ô?ïéómdKH?U‹gÿ–Ý?f'v˜ðH?U‹gÿ–Ý?ïúWbE"'?=Êô2Þ«¥?F¢uýøÍ ?=Êô2Þ«¥?ïÙ!—)|Ñ?€Ô%á¯ë'?so4ˆOR?€Ô%á¯ë'?ïèm­«Q?tüQÞè­Ò?g'SÔ'?tüQÞè­Ò?ïÖ!ý"L}?iæ*iԐ¬?tïwÑ5?iæ*iԐ¬AGN4FGL J0322.4+6606?æ<rՓ#@Teè'%1À:%½›¡æÀ;¥KJ-'@Ri|ñBM@TÓ¥¸?Í%ÑuÓì§?Â(ÅÆôÄ?÷¡w´l"@mËÑ¥#»?ïƒß=g¿'¿ÌŠ|ºe¿ç
@/p¿ê¬t½—$ʿ竊\å´$¿ïòªa½à AGNbcuLQAC 050+066?ïþ_qT«ÿ?"ËE +?*楿K?"ËE +?ïíKJ´·¶?eُu¢È-?b´µaEÊ ?eُu¢È-?ïʌÝâÊ?y'ôåÚp?z¹'s¿Ç)?y'ôåÚp?ïì˜6Ã
¬?FQhÀmIÙ?cgÈùœü2?FQhÀmIÙ?ïûA¡??»œ™Ôè?BùÜ»8??»œ™Ôè?ïL¡nO>?•8¾ywæ?kɟL?•8¾ywæ?î±ü27‹?žn£.©ó?¤à7
HÒY?žn£.©ó?ïŽwK³T"?whfŸ0\?Œb-
/h?whfŸ0\AGN4FGL J0322.6-3712e?ÅùGÿóìÀLX±mÀ9ÍàöO}À<Oʪ³Q@ÇìÀ24±@9‹q¸ª?²ðìçŸ?¨)>'·Ó?ö U?Íui@¨ÕzÆDÈ?ïZeÁû¸s¿´åcË+¿â³KQ7*9¿âÇÿÞr¿¿á>ÀÚü¿ÝŸœèÙrÍAGNRDG3FGL J0322.5-3721Fornax A?ïü/å;?.3äŠ`ó?;–'i ‡ä?.3äŠ`ó?ïö‡M^$?Qìê?¢,?Rñe||)?Qìê?¢,?ïð¨Ì½]n?bñ‹‹†Í?^®fåz3F?bñ‹‹†Í?ïìtaÉ*?LM$úèWË?c‹žCInE?LM$úèWË?ï÷ïÛù8?F÷L"š±?P HÖÞ¬?F÷L"š±?ïÚ7\@P[?tÏ,Õ×Q?räQÝÈ£?tÏ,Õ×Q?ïßÅpô*?y÷J$=ƒc?pGž°ï?y÷J$=ƒc?ïÁÙ@Z—?k¢ƒÑÇåˆ?@>&ˆØ?k¢ƒÑÇåˆAGN4FGL J0322.9+0940¿î@g'û	ÀCŠ'¥aNÀ:ËW´ûßÀ<$ý~E€=@òÁ	J+@1fàé´?ƑཚÉ¿_Œ‹Û?¸*žd.©?ÿ›£4"¿î
ÍHÏD?ÌfH'ZŽ¿æs½œ®!¿äYQªí¿á.¯½µƒ¿áìà¾q?]AGNbcuMG1 J032256+0941?ïýE9bã?)ž^|ÆzÒ?5Ö6Û½x?)ž^|ÆzÒ?ïôG°BÓd?^vÛOÛ®<?WpŸÕç?^vÛOÛ®<?ïãז]Á?lý"ïz¹?l(irã¶ï?lý"ïz¹?ïõ÷´?;‡e.–âù?T÷ÔVf¼?;‡e.–âù?ïô¶Ñ–hÀ?S‹>
k×?V']gO1?S‹>
k×?ïϔ šC?{?>ê?x5üáD'?{?>ê?ï»!Ææ7?"ËšoBÞ?7½u¾U?"ËšoBÞ?ï²$ÖVÁá?vÔ,· ð?ƒvÊ{%™?vÔ,· ðAGN4FGL J0323.7-0111¿Ï»؃hÀFœÙ¾L×IÀ9y|"MÀÀ<ýð[GN@²S~'<?üöñý2Æ?³†þ6|>?¹ œ,ÆÝu@ª`%څ@ã‰û÷Þ?ïÿ-<y-¿ÅƒÙ¾Í±¿ßúTvyÚ¿ÑyzϪ¿å†Ö]ð 9¿Õ•:¤Á•âAGNbll3FGL J0323.6-01091RXS J032342.6-011131?ïüoª\àV?0åÛO¤Æ?<'«·tÁ?0åÛO¤Æ?ïêüÊZE‹?gLý§:¸?e5©Ùýh?gLý§:¸?ïë
<~‹v?dSÿy³?dòÃo–'Ø?dSÿy³?ïzÂ9(ž7?r¡L!0ô4?§¸Ù4k?r¡L!0ô4?ïù¬i]š?B†kͶçó?KÍMjKNª?B†kͶçó?ï¶/ZOq?†Ÿ‹?›R?'t)‡2ÅÂ?†Ÿ‹?›R?ïÀŸ˜iÌU?'^¨ôTÌó?°3ÞW¥`?'^¨ôTÌó?íôŸ‡dU?—_ö,;?°[Ç4ÝW?—_ö,;AGN4FGL J0324.3-1313¿¹ŸÝ€y7$ÀIÙÕ<ÝÖàÀ:ƳÑSDKÀ<rºÇË)@¾Z.t²"@l'	Z?ÅÔú˜¸?¥CÃW®?àLS?È@f¢$'–H¿Ñ-!¡:wË¿æ<¿ß®Q¿ç/SàQäÏ¿ã§CÁð`¿êÖ
ˆ~¿#¿ïþašNË?AGNbcu3FGL J0324.5-1315NVSS J032430-131002?ïùéäÆÏÄ?Bœ)hµã£?HXmàŠµ?Bœ)hµã£?ïõ¨–6¸¤?]»¤ë¹g?T®Ó^T¨³?]»¤ë¹g?ïÙø¬Y?yè‹72Ê?sƒ¦·ž?yè‹72Ê?ïù W¹Ol?1·KÙP6ê?K~¢!ŠÓ?1·KÙP6ê?ï÷pÝÁDa?J?sñ˜ˆ…?QDþ¨6?J?sñ˜ˆ…?ï׳¤Ìlo?rÙÑBbÖ?t&-•ª@Å?rÙÑBbÖ?ïå$f´'?q(
Üu'?jۙ"¹.?q(
Üu'?ïØ}ýSIË?byÑ2N:,?sÁE-_?byÑ2N:,AGN4FGL J0324.8+3412?Ì7ôß¡¡âÀ2¶®::ŽqÀ8­<Íè«À;±5WСn@—#ȇ@)@k*?¥ ‰ª
Z?­‡½Úy?ÿÉóÔx"@#ò‹ù
¿Ù뎃æÔá¿çöÌ ,/߿ꉢ«'â¿éSÐ↏¿îcó¯5?äÆ@–žAGNnlsy13FGL J0325.2+34101H 0323+342?ïþ]
LCÐ?#¦ùú¢£?*/(ª@ð~?#¦ùú¢£?ï÷ON5±×?R®kÁLć?QacDåa•?R®kÁLć?Q¥ I?‹×"‹?˜+¤V]›?‹×"‹?ïÿ
r"?"%Ë݆?QÂjd2?"%Ë݆?ïýØ-±œ£?400Æï<D?1>'YÐùG?400Æï<D?ïÚ%@èc½?vñp0™ÄÅ?rí_yð)q?vñp0™ÄÅ?ïw˜ú|!R?s"Á³Ú‡?'à·[
§?s"Á³Ú‡?ïûî¾96-?6©º—èS?@E¨ý"n?6©º—èSAGN4FGL J0324.8-2043¿ë™ó±	š*ÀK?™ÜµxÀ;hi²KAGÀ<ÈõZŠ@ "¤Ht8?鏂¿b€ÿ?ß>P}pï?îøÒpXƒ@i΀+3Š@	î…äÛâ>?ïùÈþáòÏ¿ïñ"ݝ)œ?ëÈòíÈÅ×?µnTœdz(¿åvpnö¿ïÿÿ" 5•AGNbcuNVSS J032451-204324?ïþ6ÿû´?(b˜"$ù;?,—ÿã®^¾?(b˜"$ù;?ïõÊu7B??ZŠßº‹¼Â?Tk€ýaÜ?ZŠßº‹¼Â?ï¦	yëÌ?&"3`ìˆ?†}¹èdE?&"3`ìˆ?ïón?NyöP›s?YãÉO×2?NyöP›s?ïþÌ£ ë?'†¡õ©©ù?#5ÑúºÛ?'†¡õ©©ù?ïÙgyaã?€¼š?sLxâëvI?€¼š?ï¼}æ
´?ƒ8‹v¾?€à†y"‰?ƒ8‹v¾?ïú|ºÕ?HÌ2íø§2?G›áÈé7v?HÌ2íø§2AGN4FGL J0325.0-2416¿ï›ð›½ÀK³w ÈÍdÀ;[s¶±•À<µ\ÿµ@ßý®ÁôØ@]SG¥°ÿ?ÂÔé¦Í3пµ×"z,?òã<æ:\@hNAy¿Ìb{ 4hg¿è÷ÿ¶.$Ö¿á•+uϏö¿ïì;ýÝ?퓟ïôð?Ì7
Þ:ŽAGNfsrqPKS 0323-244?ïÿ«" ê?ÒO>h#?<_Ó4zó?ÒO>h#?ï÷Ì :Ä2?R|…£yÎ?Pg¿¥ô{$?R|…£yÎ?ïØMۙÝü?yênéÚ´?sÙÔr8?yênéÚ´?ïÿ÷uS${>ÓúeqÓPª>ч+6Â>ÓúeqÓPª?ïÿ2Ötžì?(~óF¬Ñ?¥3ö*ƒg?(~óF¬Ñ?ïÝxù]pì?toô«Z›?qCƒ;ùö:?toô«Z›?ïÔ÷ƒHŸ?~Úç÷ 
?u"qB{8O?~Úç÷ 
?ïÿ9ö4¾è? Ò°˜ g?Á3†>Õ¦? Ò°˜ gAGN4FGL J0325.3+3332?åkÝðEÖÀ32|EÀ:ۘkœ0MÀ<(ŠÅÁ@@ÞÜØÞ}ú@Ñ1ìVu?ο'½†,?¾¡Åg}¾?ò¢}SõÌ@Êãés÷t¿ïð£5úÐ?ïýâƒî6ª¿ê¾ÝöÀ¼¿ÃË`æõ—ò¿æ£Ò½§•Ü¿ïÿ'ò¶kaAGNbll2MASX J03251760+3332435?ïõÖ³±Ú?ˆŠ"¯T4î?TSÒ'éË?ˆŠ"¯T4î?ïîŽýÎ^?a³û`"2S?aqf)²-?a³û`"2S?ïÀµe¹('?›ÿ·õ?¥M/cE?›ÿ·õ?ïÞîRX'h?U™,ìé˜?pˆÖÎçWà?U™,ìé˜?ïÝcÉå"?za,d:Ô?qN)›Á§?za,d:Ô?︈ç½
"?ˆ|p
æì?ÝÆŒÒá?ˆ|p
æì?ï¼'†Å?—›ª$ˆç?œfÏïv?—›ª$ˆç?îñU#·®ò?"mú"~+À? ê­Æ<ÞÚ?"mú"~+ÀAGN4FGL J0325.5-5635?é†ÃѺÀHé*0U2aÀ9ÞT8fxÛÀ<c!¸·l@¤&ó?þä¡Õ¨>?²@ÊžUì?£Sþk«?òTE·š5¡@´2vÐ?ïÿ˜ È¢q¿ß°Å/Iš¿ÜÚ\FQô¿á3ËÿY˜¿ÙÏ:û©"¿Ü£¸AGNbll3FGL J0325.2-56341RXS J032521.8-563543?ïÿ&]¯*?
¨v¹2½Y?4JÆB˜µ?
¨v¹2½Y?ï÷ýõ[-Æ?Pšò§UX?P–›´?Pšò§UX?ïõϹÕèï?^þÒg#L?T`‹Û;âœ?^þÒg#L?ïþW½geP?C—sª{?*"-C8ì?C—sª{?ïþҗMJG?´u3În~?"֌]`?´u3În~?ïàß"XE?qWwé¤&™?oo ngk9?qWwé¤&™?ïósi¦"0?h•¸i`'L?Y-1i??h•¸i`'L?ïý‹Ä]?)X	™%Ç?7#£Cºûê?)X	™%ÇAGN4FGL J0325.6-1646¿èøáZð´ÀJwÃ?…Q
À9'BG£-À;æ³ «Ü'@¡ØR¼æP?üÖ#l?¬bjBD¸?ª—ÁA;J@ìsƒ…[@
sd{ª›¿ç=†É2¿Ôëˆy¶¥C¿à-qÊÛ[¿ÔOóÞ3§w¿âEœÂC¿Ñ,`Eºõ4AGNbll3FGL J0325.6-1648RBS 0421?ïÿ,ÿΓ?l›¿áva?`.´æ?l›¿áva?ïö­±SŸ?X–4þ\?R¤¨wÐí?X–4þ\?ï÷جÝvÇ?;£‡=¨Uj?PN¦E卿?;£‡=¨Uj?ïü4U¿q'?)±è»"tŠ?>]P©YH?)±è»"tŠ?ïþÂášö?[åŽ™?#Ñäí!à?[åŽ™?ïÝ%eñÕ?rJOÅh<?qm7®™¯?rJOÅh<?ïø¬C¡"?[19â耧?MO‹©¤þ?[19â耧?ïöE÷°ü?G~¬";²?Stځ?G~¬";²AGN4FGL J0325.7+2225?îkÆ£ªYÀ;ù@»±òVÀ8¢ÆÅKÏÀ;Ä"Ÿg8ô@G¶h‡Rð@K%}h
«?¨íöëÁÉ?ÅdI,@öøj	‰@²ÑÖKý¿Ø1—׿¿äª¿_»ý¿èwÓ«äù¿ë,L$Ì¿íîa«ì¿ïÿíöé	AGNfsrq3FGL J0325.5+2223TXS 0322+222?ïë#«ðx?c"ýSaÙ?dÜSÐOß?c"ýSaÙ?ïî†-Îg?duPds~q?a÷yó-Ù?duPds~q?ïMu·Mp?'Ð,"Û¾?–_±IR?'Ð,"Û¾?ïã{I™Éb?Vɍ³'?l"¶›Ð†?Vɍ³'?ïÏó;Ì_?xAo¶B.?xtLÌ<©?xAo¶B.?ï Ùpìs©?›ü3`¸N&?‡É£·$¥ï?›ü3`¸N&?î¾³·ò†?œfCtהè?¤Æ'ðs–?œfCtהè?ï3I¿£?ŒúÐÁ# l?Ÿ]™' ¡­?ŒúÐÁ# lAGN4FGL J0325.9-1843?ê'ñ¹|tÀJ̹#¢œxÀ;³"â{À<‡¡†`@aA¹^@£BàO`?ʕΈ䕖?ü–"¨q?×jîöÃ@\@c±^²<ÿ¿å‰ÿ]BÑ6?ïÁÿáø¿é. À4
¿ÕHãß
>¿è^ëÈRj¿ÔX£š¤["AGNbcu3FGL J0326.0-1842PMN J0325-1843?ïþjºÅ"?%Ž{%Vô?)TV^X¯?%Ž{%Vô?ï÷æaQ`?QØè8U?P3=ºon?QØè8U?ïê›é`‡?l!¾@ÂèÈ?edþ½Á\?l!¾@ÂèÈ?ïûô_/\Ü?&nFݜ—=?@."R à¡?&nFݜ—=?ïùMcÓ?R¨՜Ž?JËþûÊ\è?R¨՜Ž?ï×ô÷Êb ?t­Ð˜ÁOê?t"/ÇÖ?t­Ð˜ÁOê?ïۜëkì?yÊMáM¸?r1õ†*'/?yÊMáM¸?ïëúk»\?V"›>9•†?dôsHcÔ?V"›>9•†AGN4FGL J0326.2+0225?½¢™×ÀE5¬îàóËÀ9RÁmóùÀ;ý'€ ¤P@ )j \×F?ý™SÃÌs?²ƒÆôp«?"¡q\í?îFTþ_@:;j?ù?êEXßÀ‹¿áp^¢LƂ¿âsEaÞí6¿Ô£,å¾`¿×²!vrM¿ãûbâMhAGNbll3FGL J0326.2+02251H 0323+022?ïþ¶'C£?k÷Eˆ~?$—Û¾½´?k÷Eˆ~?ïö—QüÞ?RšÑuÛ.?RÑ\Ã$|?RšÑuÛ.?ïöïØaø»?cH¼ëVó?R NÙÊÌ?cH¼ëVó?ïø1·ÝýL?7ˆ–²lÆ?O9¼¡ò?7ˆ–²lÆ?ïýyî·
÷?)áÕõ¬á?40Œš?)áÕõ¬á?ïÕÏ	qÞ?€¯Dn¡u¿?uxçYU[?€¯Dn¡u¿?ïöš¶5m?h¤ÑF‰EF?SÀÊoÙ6}?h¤ÑF‰EF?ïïXøa?M–¡ßvIÑ?`§'«B?M–¡ßvIÑAGN4FGL J0326.7-3404¿×0òš¢êÀL	U`"¥À:ÖõtŒÀ<Æ$)ªô5@^ê˜Õ?þb,•Š@`?Æ(¿ý0—Í?É(Äûb7@C]œ"I@éj£·Õš?àMÍþ¦
Æ?â$EÅ.…±‡!¿ÞÉÖço¿ìÏ‹¿¼¿­"ŸÚsAGNbcuNVSS J032644-340330?ïöa
±ß·?QðøN#…?S=ê–Á2õ?QðøN#…?ïôÞVë|Ä?Tv(J&â¾?VCR9"˜B?Tv(J&â¾?ï_†»ùôV?‰è‹kÄÏF?"('yCB?‰è‹kÄÏF?ïáoËXÈ2?TpÀœ¼³€?n4‡›f5?TpÀœ¼³€?ïÕöLŠX?wSCˆ8ÈÇ?uøaI÷¾?wSCˆ8ÈÇ?ïÕ9
ÎÛ×?wΈ˜þ.¾?ucy*pt?wΈ˜þ.¾?íÿ#³Ö?¢¡7—¢Ç¶?°ç9ó\R?¢¡7—¢Ç¶?ïªð
ïÙ?s	Jþ•?—?…CüŽn]Ð?s	Jþ•?—AGN4FGL J0327.5-1805?òÒߥÀJrGE8ïÀ9þ\XÆj³À<3ë‹Ô´ù@ñÓ"§IÛ@‹ÞZ"ÊM?·Ý­DÇ/T?¹@1¸#?õõƃÝp@Ä E°8m?§9ÓtÝ¿è	N}'{=¿ìòwéF¿ãˆ$&Oõâ¿ëñ–¼ˆÝ¿ïþùÀJÞKAGNbcuCRATES J032743.34-180342.0?ïúÑjÉÖ??Âp£Ä4?DºUË¥ø5??Âp£Ä4?ïöÎÕg®?SÖ5Ye»]?RbT´9do?SÖ5Ye»]?ïÀì'/µ?''iOšŠ?‰·qÄZ?''iOšŠ?ïþn§Ê×!?Ëë%aBH?)€ŒE??Ëë%aBH?ïú>`
?Cè×u?m¹?G«£®¹wË?Cè×u?m¹?ïà«NLê?pÎòxLQÆ?oT±Í2ôW?pÎòxLQÆ?ï³yXuPÔ?ˆ4ø¢lÃ?ƒ!©ÞŒC?ˆ4ø¢lÃ?ïøêHC÷¸??¦ÿf}߶?LVÞýRÔ??¦ÿf}߶AGN4FGL J0328.8-5715?ØÝ[p5rÀH‹¼¾aÐÀ;žJœ	¶À<ì^ª°BS@"t˃÷q?ñ×ôH;Ù?äoñ•1ä?á—Ïà'~@˜"?úJVËhɘ¿ïå¿Â£(9?ï–Á¥)ñ¿äÀ€æDm¿Å3ÃçJýT?¦à±[,K¿é}"€U$öAGNbllWISEA J032852.69-571605.5?ïüh¿9ÄÐ?7Ȳ׌5?<ºŽÈÈ?7Ȳ׌5?ïïzÔ)ý?fXêâ=u¢?`…+B"Ÿ?fXêâ=u¢?ï«Kî¿n?zÑG91Ed?…->P$c?zÑG91Ed?ïñûùh¿»?Qyj2¤q?\
bºš{?Qyj2¤q?ï÷Øñ•¦g?U|ÂëñÙã?PN5»\?U|ÂëñÙã?ï âM½x?›|ʲ¿{?‡Çl2]>?›|ʲ¿{?ï¶Â¯ðü‹?'\u§ñþå?'OT¯ÙR?'\u§ñþå?ï1L9{?y"Xp2±?~·çhQž"?y"Xp2±AGN4FGL J0330.6+4659¿Ã¹TæÐôÀ™tNƒÀ9•¶åû7À;ÀcK(ó>@<8?Œˆ@oÐ!ëã?¾ÿ·ZʦØ?Ä/â›Á-@Ɣ‰`[@g+Þ*B¿Í—£ö¿åz¡–'õ¿éÎÚÄT®¿éêÿR[§¿ïóȟ@¢‡¿å¶]õ~AGNbcuB3 0327+467A?ïêòŽl-¿?iÉ×=ØÂh?e
q'rh'?iÉ×=ØÂh?ïØ }ìóf?w>‹@wï?s¯Àöøhá?w>‹@wï?ï­lCcñ±?|¾v¢?"¤ï4º?|¾v¢?ïz#ç)´?sèFn-?»ƒ!¨´N?sèFn-?ï4!š%ýã?ž8	Ù3?™{̼ø¡?ž8	Ù3?îþ'ºõVP?¨LÕ¼M? äRbhú?¨LÕ¼M?ì¹3Š`?°]KÑò?¿¢7Öc­?°]KÑò?ëÖÅôì?ªÃ†F?Ã㔤è,O?ªÃ†FAGN4FGL J0330.6+0438¿ìÙGÿóë ÀDã>ÿPÀ9Ï"M1âÀ<%E«Hï@»ƒú @DÀßXÀ‹?º½<áÝ«?¿C¥`$Õ@»­À˜$@十×?ì۝_¡Ñ!¿´&,9™Ô¨¿æŸ³%]¿Úþ$þ½	á¿êý՞,¦Q¿ðAGNbcu3FGL J0330.6+0437GB6 J0330+0439?ïû¿jl8?8@ÚOUÚ?CåCž'?8@ÚOUÚ?ï÷_	й@?Rl‹±àöm?QAë×ÜÏ¿?Rl‹±àöm?ï»Úć.?NdÑã¥h?	N×­<@?NdÑã¥h?ïøٖÅåä?5ün¡qæL?L™¥×Ï?5ün¡qæL?ïðŒS¤±"?X
ÍÂnæš?^çX[ç'†?X
ÍÂnæš?ï؁uOQ;?u¸uÊØç?s¿EPÈ>¦?u¸uÊØç?ïr	Þ›=?Ž›Ö1?'¾Íß.t?Ž›Ö1?ïî?E» '?PÿN¬ñÈ'?aÀº‡L?PÿN¬ñÈ'AGN4FGL J0330.7-2408¿ë½š£7…±ÀK82vtÑÀ;b«ð´2¢À<Ù£€£(@ *Ï·bØ?úM "Ú?Ôä< DXŸ?Ïpk"ð(?ûãèrDÁ@ƒ¼|±¿ïʒ€Ê÷?îrE ¿×¡P&kú¿ÒtZÅÉM¿æzÐKŽ¿Õ>ê šªAGNbcuNVSS J033050-240612?ïý,_É¢?'©E2dþ?6G¼Ò?'©E2dþ?ïò…‰tæå?a­VË¢Úþ?ZôìÖùe£?a­VË¢Úþ?ïß!—vÌ?b£¸Ý{·?puïHâAà?b£¸Ý{·?ïç¨aCÍñ?O²Òñ/˜8?hWž›5Îã?O²Òñ/˜8?ïûèj{ã•?:¸Å5üIá?@^Vô—ºÇ?:¸Å5üIá?ïğ,^5s?ƒ÷֟Œ2`?}°iÉV"‡?ƒ÷֟Œ2`?ïÛrÇóŸ?u?•2žï?rrÆ­ä(X?u?•2žï?ïœÄMf)?zÄÞmë_?ˆÎì£ß?zÄÞmë_AGN4FGL J0331.1-5243?áµ·š4äÀIsüC²Ý7À;&ê«Úä¾À<ÃNÂò®@H‡r¦@yýåsŒÀ?÷øX$Ú¿š÷•ì¼?Ô©S æêÛ@É(Åñç9¿ß˙‹í¿âþP",O¿¿é'A¦"} ¿àXÍ¡ˆü=¿ïÿý±q&´?äQªí~ôAGNbcuPGC 013066?ïýB=<L?9'ÑÉ÷8C?7…îˉ®?9'ÑÉ÷8C?ï÷]ñ&¦?Q1pY¿?QDß4"'?Q1pY¿?ïæÑӜʧ?cY°=ԅ¬?i.,§í‰?cY°=ԅ¬?ïþS×Ö?©®iÿ?'êÈ#Ëʧ?©®iÿ?ïúW»ípJ?OQ†*]?F¡x
Â?OQ†*]?ïÛ|$‡…?sz®(e?rAúuKau?sz®(e?ïÚY•Z´?xfÖÿr;?rÓ?M_é¦?xfÖÿr;?ïôýMÑ¢¨?N‰XmªY?VdÂ04?N‰XmªYAGN4FGL J0331.3-6156?ëÛÀ8GwÁÀG(µÃ›Ë£À9Yėt%À<Jè:@X+ü2@?ÿbBw†?®™½
ù#?°êÀŸÃ@¥:œ´M@¨]e‹Êú¿×û_1hÙ¿~‡€££¿ÞÖtD¿áÀmä	)t¿áæ!‡+¿ã˜r‡ÜØ´AGNbll3FGL J0331.3-6155PMN J0331-6155?ïÿámî›?ýLÏáâ˜?#˗»vU?ýLÏáâ˜?ï÷3™=Î?UB.³‹¾?Q˜Í·ÈtŸ?UB.³‹¾?ïô›•È(Î?`%IÖ?VÈÔø´)?`%IÖ?ïùñañP?3À!:ðJù?H:x¼|ç?3À!:ðJù?ïþl™¨ª{?¸™_»F?)6gÝKþ?¸™_»F?ïÝTŠ×ðþ?~ƒ}N?qUº˜ÖôÄ?~ƒ}N?ïòOµ
Ø?m"€ää•?[`•{Û£>?m"€ää•?ïïÊÛ°ëE?P^»×'1î?`5$[sS?P^»×'1îAGN4FGL J0331.8-7040¿éâí±¯÷ÀD{tÝÛÀ;ç&ďçiÀ=©'^aµ@"ÙJb¤ºà?Î*ÚI7+?ì?»×²?éóœDnÄÚ?ýâ©Ô#Ù@í§d2"¿ï÷[0H¿ïOµIùHV?ïé !óð¨¿èÝV‡Ì¼?Ó¢=ëó¿ÊAÜCbUAGNbcuSUMSS J033202-703952?ïý
	±bA?5åŒO~?7—³±–Äê?5åŒO~?ïöößoçš?TmæÌøø—?RA"ð|ù?TmæÌøø—?ïeú8sl'?Š×À°Y°"?"@¸ö¹×¾?Š×À°Y°"?ïÿ:i¢è?K0¥Y-?²Ë0G_Ý?K0¥Y-?ï÷¸9܉r?U8wÍE0?P‹ÐºŒh?U8wÍE0?ïÜr"´l?~äН¾v±?qƶ""…Ú?~äН¾v±?ï`êOƒd¾?D®#ÍL?"â¶E?D®#ÍL?ïÿ1H¢[4?%[¢›òú?ÖëiÕ-Õ?%[¢›òúAGN4FGL J0331.9+6307¿Ã•žð©@Ç€¾À9*æ?d™ÞÀ;ÎÔ°ÆÜÉ@×ÍKͳÒ@4dÁJ¸‹?²vNÜ±œ?¶Mp÷ê@WZYèª@	¸¡"Ä"¿Éëð¾ïi…¿âLð=ë¿Þ[^Ëgqÿ¿â‰Úßµ¿âú1T5â:¿ÔHþ¡†"AGNbll3FGL J0332.0+6308GB6 J0331+6307?ïý­Œ¸0?&¤‡XÇ®M?2"˜+̛c?&¤‡XÇ®M?ïåZv)c7?p7‡Tj^ò?j¥‰–!l?p7‡Tj^ò?ïðçè9Ã?iºæ+˜H?^ä0°½È±?iºæ+˜H?ïѨQ å?_JÞñHŸZ?w+×€.¡?_JÞñHŸZ?ïúôq›<¡?;?ðÝÒ?D.8—Ðtó?;?ðÝÒ?ï1	Šل?£ØœÊâ£	?™Þκµ3ƒ?£ØœÊâ£	?ïê锝u5?poþ Éýy?ek]jã?poþ Éýy?ï7¾=›t™?"}‡Û¥.ƒ?™8Gjð?"}‡Û¥.ƒAGN4FGL J0332.1-1123¿îJ¨hЊ-ÀH–s-õÑÀ:Õѧ' ÖÀ<lšu%F@¢Ä—ôþÅ@´L{՝?Õ%
¦w?؆B#æäü?þÚ®½M$@Ž¬7+¿î9_^4i?à°ïÁÄ[¿á¾Jô°¿è¸uAË|¿ïþ0Q×c)?ïÎ0Ö¯ÐAGNfsrq2FGL J0332.5-11181RXS J033223.2-111938?ïøTl‹:þ?R'¼ð|¥{?N®Nƒ ?R'¼ð|¥{?ï÷Ƒ@Ò?P´ù€6א?QÀr®Ã¬N?P´ù€6א?ï>/¹^¹|?‰'ŒlÜãu?˜:й4w?‰'ŒlÜãu?ïú¿ûÇÐÓ?3àëÆ™C?ELM"`?3àëÆ™C?ïõ
^Éu;?dn7y쐚?UåBë‡*?dn7y쐚?ïØ¥Løxš?rÎó‹-I?s­Y  k?rÎó‹-I?îÚÝ8Õ´}?–8/ßx?¢R,p4?–8/ßx?ïáhôêq?d'm·²Ä?n—í?d'm·²ÄAGN4FGL J0332.8+1557?íËu¥¯¸¦À?È)ˆ;£À;H™Ì¢ÛÀ<ŒÎóº1@ fWÎ.å?úàSý®(?ØÞG ÏÄ?âc¶ˆ½©C@ úÄV܆@ü0à¿íèÐ~]($?ïÙQu=™¿?…Ñe¹¿Ö—¼Ô¬j¿è¦¸f
{¿ïü¬ÄÉ%AGNbcuGB6 J0332+1556?ïñ"LÞÞ{?uRc3Zè/?\÷fH
˜?uRc3Zè/?ïÛމHú¬?|¸°®Þ£-?r»lÉô?|¸°®Þ£-?ï‹H¾¾IÛ?öʤ4ò`?-ÐIŽQX?öʤ4ò`?îõ¨'۞?ˆ!N‡·ß? ¥}Œ'#?ˆ!N‡·ß?ï«Æšƒ¤e?‡ çÁų?…Y[§JÑ?‡ çÁų?ï¥Z@y~?'ö¶|¿žZ?†©oëïS•?'ö¶|¿žZ?®·ãÝ?U'uìh?¥e¥Û9?U'uìh?í§&Ý0ê{?¤ÐAx?²ÆÉ柧?¤ÐAxAGN4FGL J0333.1+8227¿éðXBƒ«@5IPüqÖÀ:ÀAFmDÀ<¬Š‰[]õ@™Têèí?þC:sÆ?Æï¡
+b?Ëyˆ'!@®ŸÀ@.وœò¿îºadw?ïù·a*½C¿ä<Í`pƒ ¿×H¢L@¿â¦wÎm·¿ïㄟ6'AGNbcu1RXS J033208.6+822654?ïúj+Öó?<ƒ‰Ûã ?FWTb¯ë"?<ƒ‰Ûã ?ïÞwOþ×?pøÊJ?pÄXq)·?pøÊJ?ïáKà[Ón?eõ—?Ðç?n´‡OÚ$?eõ—?Ðç?ï»×È,?aA"³zè?

øI¨ð?aA"³zè?ïô׆ SÙ?Pt²WÌ1×?VPò@æ®W?Pt²WÌ1×?ïV҇v×M?¢öȔpõ=?•%¯
EÞn?¢öȔpõ=?吝àgM0?ˆ'CYÔ¯0?†‡ßM|?ˆ'CYÔ¯0?î©q,VäØ?'x¬žr|?¥hí=%g}?'x¬žr|AGN4FGL J0333.3+0233?ïóàî²ÀD~~¡ÆÀ;a .QÀ<‰<
ÍH@ GRBBÖ?ú{R¡ƒâ?ÒÁÐÅTÞT?Ôø'Äj'¼@Œðs›O@¨¾vÁ¿ïþÃÎ!a?ïò¦Ey†Õ¿áËZ§ƒ¿¾p¢ÕWŠÖ¿ëÁšÀ«¿ÕÝC<•²"AGNbcu3FGL J0333.6+0233NVSS J033321+023110?ïûMºâ®O?Aäw×?BÉsC{?Aäw×?ïô‰\éº?U'$ÀË`?VíFƒÜ?U'$ÀË`?ï;—qåå;?"@´µ…²?˜Á‹Š"?"@´µ…²?ïêK52'Î?PDÃZ¡ê@?e´Ê–tr¯?PDÃZ¡ê@?ïöÔS•Ï?Q%ô;Ö?RWZ'qé?Q%ô;Ö?ïÒÃog'?€¨ §Ê?výž%ðT'?€¨ §Ê?ï(;€A?'ëV¡~>?šøœ\¸)â?'ëV¡~>?ï©O1k‡ã?zø^$öU?…¬3¥'?zø^$öUAGN4FGL J0333.7+7851?Ɲˆ
>â@2vF¿2/À9ƙWTz¬À<f£ÝÀ:@Ôµ'"™€@ÐÞªDã?³PSÕj*@?¯Cûq??øùìU(P@æ ‡4U¿àQž®+w¿Û˜0bôA¿â Ð$p!Ñ¿ÜOþ$ކ´¿á‡_<ü`¿è´À}‰AGNbll3FGL J0333.4+7853WN B0326.7+7840?ïüź=?1½Ž!†Ó??Ò'p'?1½Ž!†Ó?ïî`†8¥?dV\øèU]?aŸ~³€Ê½?dV\øèU]?ïñÖ]³ÿ?mp̎ië?\SDÙú`ò?mp̎ië?ïÖl?»¤(?\†)ãã?tÉà Î?\†)ãã?ïöâðz§?HX€ši›'?SÒ:òE?HX€ši›'?ï¹I%xF?†ë÷™ÛÝ?­¼p"x?†ë÷™ÛÝ?ïèaщӇ?u–U0¤Þª?gž.œ¨H?u–U0¤Þª?ïa ŠéAf?€4"*ÂWp?"Ëî¦Go.?€4"*ÂWpAGN4FGL J0333.7+2916¿îþü°üHÀ5êÝYÀ9óæí	ƒÀ;­	¾º@U‹DÂ&×?ýV‹@š?­[åÂâØ?¸Ñ|ŸbÜC@‰Oâ–b­@—Ñ)(¿Æ­þÖ_G¹?àµbîᶿޛ¤¡4˜Ž¿Ø?"Š¾µ¿äg8ô=T¿â;ÊYêWAGNbll3FGL J0333.6+2916TXS 0330+291?ïýRA§{k?*ˆñ*Tè?5mò3÷'?*ˆñ*Tè?ïë7l0ˆg?cˆ²Þ\ó?dȓ®{Y?cˆ²Þ\ó?ïß©Áãm?s‡«'þ?pp«>ª±)?s‡«'þ?ï"%«­½?huNHPé_?Šö•{H°?huNHPé_?ïö5ub?PÚܨPq?S•ÝÃYLs?PÚܨPq?eˆÅâ?Š }Ës5¡?ˆT&¡>#ˆ?Š }Ës5¡?ï¹Á¢ï{?‡lï0hÂP?¿Ž­E?‡lï0hÂP?î![žu¡?"Û£—XÓ?­êCجZæ?"Û£—XÓAGN4FGL J0333.8+4007¿î"®åÓ{_À)Á%µ¿jÀ:žjÇ7#À<^/",z²@ÅûÍ@@yƒœS?ƃuÀÌcp?ÂK´^kñ?úOfÛl7@…íë*†¿ïôäxºüÁ?ïû+‰>¿â: D®…º¿à¸‰9˜¨¿æX'r0t¿åPJ9ßöAGNbcu3FGL J0333.4+4003B3 0330+399?ïþ?mÿ?#t™¢ö?,	·Ó…?#t™¢ö?ïñ~Å$YH?`>ò×="?]uՉÿ²?`>ò×="?ïóÌDÞù—?Ké'1 Ëå?XguÑY¡¡?Ké'1 Ëå?ïäô`ås?MR‡³÷Œ·?kŸ
Ô1?MR‡³÷Œ·?ïñû!ÙÇ?`nË­òzß?\	¾F1Ê?`nË­òzß?ï¹æ÷×x´?Š µ§ù ?†BI=?Š µ§ù ?ïÛ3éw¹†?xœÖyA´ÿ?rf3¥ÿ?xœÖyA´ÿ?ïyòç,ŽB?‡¹Ãhɐ?Á£&¶?‡¹ÃhɐAGN4FGL J0333.9+6537?ììåcœ‡‹@^ ƒxÆÀ8üƒýP"WÀ;×ÛIgR@ \@LÌ6z?þ°®‰ç?­9Cm"x?¯j*$@Á@y¸_~@°E
%W}?ìêKBž‹¿Ç
A\Õ¿Ü*¸$õõ¿áÝÖ´¿Úr
žêff¿á!ðÐrAGNbll3FGL J0333.9+6538TXS 0329+654?ïþv¯x—Û? ova6S?(•zˆÞ? ova6S?ïíŒE¦°â?f% ÿbâ?bsºp¬u÷?f% ÿbâ?ïó@ÅÔ\?`Yž¸Úý?Y~txň?`Yž¸Úý?ïóÐ4"ä?Cûq¶âG?X_–}'O7?Cûq¶âG?ïý(O)ˆå?.Ñz?͌(?6½‡ª9®?.Ñz?͌(?ït÷›#ÿ±?™¨ê–ø"«?'a›€	â?™¨ê–ø"«?ïèÐåúßô?u'⨚«?g/ô¡ë¶?u'⨚«?ïæµÑ³'g?X÷hf‡?iJ.4ˆØ?X÷hf‡AGN4FGL J0334.2-3725?Å©öš6Þ ÀK1–¦ ZÀ8V(LýàÀ;ŠÓ8÷˜R@vz†.?þ§]§{¬?¡$Xyé¥ö?±gýí<j@«BE@i¶ÉŒ&¿Ül—B|Q_¿Ù}Ã@1¿à_ÿ¯x(0¿àªjl…dX¿ãÑ}ÁKå1¿àŸì.'ãÃAGNbll3FGL J0334.3-3726PMN J0334-3725?ïþr¼‹6?!øÍóÑmØ?(Ô3áã'V?!øÍóÑmØ?ïö¼ž<§·?T/}VüëÀ?R†ÃsrÁ{?T/}VüëÀ?ïì¹z›¸¿?aT"ê¨áÓ?cF…F
±K?aT"ê¨áÓ?ïûàæV®?-ûzí]?@|gŸø;l?-ûzí]?ïþ»`$A?¦0iHb?$IüÕ³@?¦0iHb?ïØöî‡?u†üÛ«µ?søy-ˆº?u†üÛ«µ?ïé7­È®?uZîÒëo?fÈázɑ?uZîÒëo?ïóeéÏù
?KÖ h}'?Y4,sKµ4?KÖ h}'AGN4FGL J0334.2-4008?îÑÜߝ§ÀK	ˆ MÀ81"+sKQÀ;¶½-˜½@'Y‹b@žý¼XáC?—‡>¸…:?²'T>×½R@œ
²p*5@µ‰ÐMà´¿È÷Œ¾ê¶î¿ÜãÝ Á¿ã"õ¦n"¿âáÑa*<¿æà¹(«¿è à¨-±AGNbll3FGL J0334.3-4008PKS 0332-403?ïüÝe˜­ƒ?3XRœ?9Ò}v7D?3XRœ?ïõÊ6fæ¶?[À°°Fº;?Tk"B°³J?[À°°Fº;?ïç¨ÇÎ¥?kÕÆcƒµe?hW8$üe?kÕÆcƒµe?ïÿ:‰OÜ?
aú.^±?®Ø·_¬?
aú.^±?ïþ®¤Ì0M?&#X<n5C?%¶D:?&#X<n5C?ïÚÝ'È•?€4	aȆ?r'w£-ù¯?€4	aȆ?ïðÂd¶Zg?rÑEvÞ*?^{6·!â?rÑEvÞ*?ïþ0(€–'?$W¶'ÿÍ?,ýw¶ÒQ?$W¶'ÿÍAGN4FGL J0334.3+3920¿ï	yHkS¶À*æèÑQ­À:½lŸe‹uÀ<rüp(‡@!"nPj¦'?ý1?Þ<`Ù?¾%vkí¿"7"îfÐ?Ö¨"s¿ë=@3ÈÂüê¿ï¹¾GMò?î÷L!ìŽß¿âZr¦æ‰¿ÑuºÆ"$¿å˜<8d?¥y@ޗz†AGNrdg3FGL J0334.2+39154C +39.12?ïþôï£ú?·í¼	d? ±tm£?·í¼	d?ïõ€.Û×ú?UÔ²Eù8°?Tÿ¡Ú\Œ±?UÔ²Eù8°?ïöd¨Ì'?TT€…UzÀ?S6­ü©§?TT€…UzÀ?ïö!«;`?>w.¦;d&?S½ÖÂFo|?>w.¦;d&?ïþÀÌ/æ?%žÖ –å¦?/Ãîü}a¦?%žÖ –å¦?ï΋`Äw?‡çÇPÁK€?xº@qùÜ>?‡çÇPÁK€?ïù–$Ö4f?RÛÂzûR?I§mÓז?RÛÂzûR?ïÞk	°¥F?dJ£§Žs§?pÊ{
 ¹?dJ£§Žs§AGN4FGL J0335.1-4459?Èü‹äÀGÀJwŽ}ܤ±À:¹é›9­À<z	d,ÐC@¼ ý¦‰l?ÿ¸ŸõÔ-?±êUéŸì¿R 	äôû"?œ,=mO@û5ëÊ?ïë}[‹¿Ìi"ïî¿âç&J¤‡¿à`ÃY†"¿Õ:5ÛÚð¿Þ`¸vÔsAGNbll3FGL J0335.3-4459SUMSS J033513-445939?ïþÈ0l·?5•ÐëW~?#|ö¯eto?5•ÐëW~?ïø0À^¡Ã?RGó>
?O<ÿ#ÍX2?RGó>
?ïöÖÂÞ¦-?WËsóB¨?RRyÜÿ6º?WËsóB¨?ïÿUEVÌ@?4kÏö÷º?WP$p<4?4kÏö÷º?ïýà­@W?'²Ýâ?0ú—Þ"œü?'²Ýâ?ïÚ0'|G?Z'ƒ‰ç'?rçðZ?Z'ƒ‰ç'?ï÷eMrà®?`BPq"j?Q5e\7"Ö?`BPq"j?ïÿ
™=¾?À¼%R?Lћ™¥í?À¼%RAGN4FGL J0336.4+3224¿ÐÄfñ?Œ¢À2²býüÁÀ9èT菡À;ƒT¦Ë±@ÓÝ@ß'T·?¼éÝú'Ï?ÞV›Ã'@Õ¸ÜU
@¥Í¸Úýg¿¸ó3hãi¿â1®~-,‰¿ë²¶°*Ö¿ïîªm&t?ꋪ=UËä¿ïïë L'(AGNfsrq3FGL J0336.5+3210NRAO 140?í_ž))ß?ÄÑE_Z?µ¶±
?ÄÑE_Z?ï0b¢¦Lt?«×Ád½-˜?™ó«§ÆÕ}?«×Ád½-˜?çy*}÷—?³uŽSh¨x?Ñ
«ÊÒ?³uŽSh¨x?ïì]üŠ ?daCD€ì?c¢']?daCD€ì?î 	"Ûhé?¾å<–%'?­ÿg°'£n?¾å<–%'?äs©Rý±z?Ô!J÷äÂQ?×­Z
?Ô!J÷äÂQ?éÍQM`Â?±í±œ5Nm?ÈʺÊ|÷‰?±í±œ5Nm?ë¡nÞé°?ÀŸA¹³Àa?ÁzG¤"YA?ÀŸA¹³ÀaAGN4FGL J0336.5-0348?ØñÅÌõ´ÀF—ædNÀ;Eag°À<JFu/W@"pø¶4¯à?ùìl5ç?ÉmŒàΌk?ˆÊ‰¦‡hÀ?ÁE‡ô€›?ÿ¥,ŒûÑr?ïþ¹^Zÿ*¿î' ×?ªqDC"l¿¿ÛfwBוÿ¿ÜTÙv({?»±Æ¡‡GAGNbll1RXS J033623.3-034727?ïþÒb&Õq?¥BCó½&?"ÙÝ
R?¥BCó½&?ïõ²Ì<üW?T.'É??TšggÊÁé?T.'É??ïòA±òñ?Y‰ŒP›Ñë?[}ܬ˜>Æ?Y‰ŒP›Ñë?ï÷Û¹¿?9Ðõéþ†©?PH|Påçe?9Ðõéþ†©?ïÿî€aö?+Èù_µ?¢,"%:¸?+Èù_µ?ïÔdÿgn?;KFmT?uÍü‹úõ'?;KFmT?ïòÀk·Öh?fzÏdæ¹O?Z(âÉϜ?fzÏdæ¹O?ïéô¡Ð}?XF!–…­?f_ŒÚü?XF!–…­AGN4FGL J0336.8-3612?粬ÃrÀJ÷¦a(9À:DՑ—l™À<m?æŸÜª@ȋä¥0§@[Ò#Mââ?½":'x5?—³HG8ñ?Õ螄ºåD@<¶a{p?1‹"G¿æèG]ÿ¿æ¨Š'¾Ú¿ëpê7.j¿ïøp¿…¼m¿ï÷¹_‡¤úAGNfsrq3FGL J0336.9-3622PKS 0335-364?ïùANBÇê?E÷6óŸQ9?JúÇÝùõ?E÷6óŸQ9?ïò½"&ã?\æ¼ÁH«‡?Z"÷{@ý?\æ¼ÁH«‡?ïÓmáëþý?v1Ðä´Í?vIÿÁa?v1Ðä´Í?ïáÞöß´ ?\´-"Hª¹?n!	)êH*?\´-"Hª¹?ïïp'êµ?`$ÀX'Ç?`ôkU›3?`$ÀX'Ç?ïÑ)ÞuÁ£?'E..ýÊ?wk¬aþ'?'E..ýÊ?ï¼x;z]?'é e¥Ê?€áÜ9'®?'é e¥Ê?ïa#—<{?"[?c'£˜?"Ýû‹`¢«?"[?c'£˜AGN4FGL J0337.8-1157?ߪfï*ù1ÀH
A1"¸À:ž¼Õ,À<_‡ÚTtÌ@,³‹™Q@ž/Egé?ÄaJȦ?§ß"\BÃk?á"Ì`it@Ðú'­Â?î@aNÏpì¿êÈ@Á;I,¿äD³zì¿é¨aé)#æ¿â¨:{üС¿ïø¡œZAGNfsrqPKS 0335-122?ïýE÷—6ú?1Ë´•(?5ÐC²¼t?1Ë´•(?ïó§páƒW?ZŒ_&²˜'?X±<ùR?ZŒ_&²˜'?ïÞ«Yé?p>Ù2•º?pªS-[?p>Ù2•º?ïõD)œþË?>ßú'}7Å?Uw­DtÈ?>ßú'}7Å?ïýWX£Òz?6ùömN?5E:T¯cä?6ùömN?ïÍåÂxFI?"‽!+?y
¶k˜?"‽!+?ïÅÁ%y·?€¸8l¡?}~Ÿn¢ük?€¸8l¡?ï´õD‡Ð?qŸx5-ÏÀ?'®Õܼ?qŸx5-ÏÀAGN4FGL J0338.1-2443?àñ/OgÀJNœË}AtÀ;r–ÇWBÀ<¼œe%ô†@!óx"9®"?ûp)þ×?ÉÁ`ÝæO«?©Ü½ýôY{?äáý€É¾û@w{	
À£¿ïÜT\È?ïŒD±à¸<¿ÞaÁæê°¿ãáÍzq¶&¿æð莐§?ã笁Ӫ7AGNbll3FGL J0338.1-24432E 0336.0-2453?ïÿ5Ö.S?
3¼/§ô?E8xû=Õ?
3¼/§ô?ïö¼ã~G·?U|ŠPb?R†9‡að?U|ŠPb?ïǚZ¬j?'ʝo×qH?|2ҋ¸»_?'ʝo×qH?ïøØdýÓ?>¿nófn?MˆŸv¥è?>¿nófn?ïþôÓ&-?,9<[û÷{?.@°Úoˆš?,9<[û÷{?ïÖⅤLÚ?vħwQh?tŽ½-go?vħwQh?ïºå°ÍÆ?‡ÃGÔ/5°?F¸Böxƒ?‡ÃGÔ/5°?ïÝܳ/þÜ?hûÐ]âr?q¦zŽu©?hûÐ]ârAGN4FGL J0338.5+1302¿æZóStFNÀ@w¼Â"çÀ8ÖÛjËÀ;~$–¸=Ê@ K	óô®é?ø"ËßgD?±2jáJ]?Å,Àþ7~@ßZ',•Š@=ZÿU
¿ïÿæj,Ą?ïÿô¬å¦¸¿Ô5Wû"‹h¿ÆÍ7€ÊÀ®¿ßaŽû°åæ¿ÜB"dXðAGNbll3FGL J0338.5+1303RX J0338.4+1302?ïw8%‹TÝ?¹Wn'B<¥?'ûImú]?¹Wn'B<¥?ïِl@½W?Œj''²mÓ?s7ÉÑ2ø§?Œj''²mÓ?îEogÁÛ? ÚšA"‡Ò?«®iÌP? ÚšA"‡Ò?ïÌÚçË3x?f•wf5‹?y'Œ‡ñ?f•wf5‹?ïo"L^¹…?–ü֒¹Ïœ?'
–{V?–ü֒¹Ïœ?ï'ëzÀn"?—UØL¿×?‹E!LtÛq?—UØL¿×?î¼DR/?£'n;¿@??®Ä;½G(?£'n;¿@??ï…ÏüñÇ?ðú Šª?ŸoF•?ðú ŠªAGN4FGL J0338.7-5706?ïÿNéÆOÀGþ+@öjUÀ;ø|·
èÀ=,:ñn@"ANoÑI?úç5ï¦?ËîÂÖSß%?–ï(lZÇ!?Í ÓŠ+<š@.Õ>5p¿ïî4[Q_n¿äùp~î©?ïþ$'ýu¿ÓÄ­ÄsâÑ¿êýOa<é?à@¿ºAGNbcu1RXS J033832.0-570449?ïþÓãu
?&XJÛP#?.ĸÀ
–?&XJÛP#?ï÷)ëix?S?g2¹ò?Q¬)¶$ñ?S?g2¹ò?ï·%í5´(?€_-Ýgàs?'6"¶'ó?€_-Ýgàs?ïûʬ"¦ž?5$µ$Ä?@ÕNsÛ¯?5$µ$Ä?ïþ0é=,?*uú1ˆ|?,ñiúKf2?*uú1ˆ|?ïÜõ&2CÊ?s¼NÕŠ?q…lúêã?s¼NÕŠ?ïÕ}j¹Ý1?€s›WG—?uAJ§0ï?€s›WG—?ïöNfs7?R'<ܵ?Sc3@s1?R'<ܵAGN4FGL J0338.9-2848?ê#m­Nú†ÀJ"K±¯:À:ŒAœƒÀ<^.bT@&n¿%oP?ÿ…1˜(€R?²#M"M2¿—Ÿ'ya7J?èrŸæ¿@àP64?ÁH½Þó@¿âXœ‰8#¿â@^"àÍ5¿ß	Ñeõ¿Ü&D!íæx¿ÆD
›åNNAGNbcuNVSS J033859-284619?ïþû‰+jð?3áІ? GlqÏàË?3áІ?ï÷#Çt7#?TèÓ×Հ?Q¸qÄHÏ?TèÓ×Հ?ïúÛM™?0ޔéxù?D'ÉÃẶ?0ޔéxù?ïÿ<!H"?sà[	ã§?}!;yˆ?sà[	ã§?ïþ¦®L{{?'돝í*?%•ۍÈ?'돝í*?ïÛÃH¥Ça?s&$:r›Â?r[šŽkÓ?s&$:r›Â?ïûZqïI?T;ÏK›¡"?B–9@ªr?T;ÏK›¡"?ïþG$›"š?[¯¡Ü¸?+·QËOó?[¯¡Ü¸AGN4FGL J0339.2-1736?çћ̂W¼ÀIG"#ÐÀ9•²F8ÉuÀ<\ªûÁ­@†rK!œ?þd¨Uôÿ?°ÍÂkØ?¡ØÎbÏ1?ó'
8ͦç@w|üTú®?ëpø@¿Ð‰§»§¶¿áC™b<5:¿Ø´Ó[Ý '¿àÇ7—FC¿Ý6¤!1þÖAGNbll3FGL J0339.2-1738PKS 0336-177?ïþ¾ÓK'W?¼´eœå1?$ʳœ?¼´eœå1?ï÷jUfíS?Pi"Á®Ö)?Q+U—ÙÊe?Pi"Á®Ö)?ï÷ÿï¬G?B6+)?P"'
¥d?B6+)?ï÷kÈa>p?8ðÑG¡ëÃ?Q(nöAH?8ðÑG¡ëÃ?ïý°6?&ÿóòJï?2-Y»?&ÿóòJï?ïÚµ¶¹Bµ?tÿ½±ò?r¥$• 5¡?tÿ½±ò?ïùúºå?Uo
†}Áx?Høi½™¸?Uo
†}Áx?ïìô!Fîô?Qh-EEtø?cÞ}÷Ä?Qh-EEtøAGN4FGL J0339.5-0146?ì&ֆ½|€ÀE:h±šA_À7qëýê|
À;gKoj'@
Qg¦­S@ðÜá?'Ö•<VŒC?´Ý)¼<ë@kMHˆ/@EµªœK¿ËûŸú[Ñ¿àÍìlø¿å€…áÖÊ'¿åÒBW"¿èæWbg~>¿ç]™£ª""AGNfsrq3FGL J0339.5-0146PKS 0336-01?ïæÔ¤Ýþ?'q
8–­(?i+[ªI	÷?'q
8–­(?ïñ‹hS{}?gýFÊç/Õ?\é/‡Ãµw?gýFÊç/Õ?ïÌƌì·ú?€5N˜uÌp?yœ¹ƒt·3?€5N˜uÌp?ïþ		,é1?#È
̒÷Ï?/olxµ$Þ?#È
̒÷Ï?ïñm'±Âþ?Yul՟ö?]$ú¬ø$Î?Yul՟ö?ïË:8`Ä?€ì×ÁT??zbãË$)Î?€ì×ÁT??ïDz2[‹±?ƒ
Lߪ"ž?|&æÙ_˜?ƒ
Lߪ"ž?ïø¼jæ#?CýìŠx?MUFúáH?CýìŠxAGN4FGL J0340.4-2422?Æ_ǦGQùÀJ ÝDÀ;ö,A§jÀ<»UãTÏ@ Oa<0?üz0bžZÉ?Ñú¦]Í;?Ù9Ã¬è@$ž¶,?ú©W³è¿ï×+Ë_åC?D8>5?łZ7Ùá¿Ö~œÚñÔ¿é5­@ÀdŠ¿ïúö`™ó²AGNfsrq3FGL J0340.4-2423NVSS J034022-242411?ïæG[g?p7ö­A$a?iëþÝÀ`ë?p7ö­A$a?ïuhϖ‰?™^|¨–8p?'Rÿ'Û?™^|¨–8p?ïQ¿ô³Vë?ŠF%r8(Q?•Èn¼Œ"?ŠF%r8(Q?î*×ì)x8?›ÙŹÊ?­R>Dc{?›ÙŹÊ?ï¤ÿ9—·}?ƒ°`G¢Ý¹?†À1¼ ?ƒ°`G¢Ý¹?ìñ×*\Ó?¿™£•¾?¸qGhdçb?¿™£•¾?í=÷7b?§¯9¸	PŸ?¶FD?§¯9¸	PŸ?èrֆVh9?µ)._r?Î4¥æ¦_?µ)._rAGN4FGL J0340.5-2118?ï¢Òj›MÀI–Ñ¿zÔ²À9E?']<À<Ciô`@©÷è‰ø@Á°9ï?ªî^å5?°0Y9(Á@'ÿœ,ñÑ@
Ê*uõO£¿¤øÜc˜¬¿à@úœðž¿äÿT¿:¿åqøÀƄ3¿à]s]Å­õ¿è ;tJT¸AGNbll3FGL J0340.5-2119PKS 0338-214?ïþ·~d'"?K!êê´Ü?$ˆ7×Ò?K!êê´Ü?ï÷Ú1©	?TËmJU?QÞK#»®.?TËmJU?ïöYi…¯?Aíú|4Å?SM.pB¹?Aíú|4Å?ïûI0è^?0žÏÈO¾À?BÛ@($T?0žÏÈO¾À?ïþ4Oñc?((z‰Ø¥œ?/¬¶É1ié?((z‰Ø¥œ?ïÝ×<3?rqq®'X?qb²–Ž?rqq®'X?ïïW"奌?kð† ƒÀ?`¨l:ìE?kð† ƒÀ?ïñ*:CÑD?Q½®~'?]«‹¤Xx^?Q½®~'AGN4FGL J0340.5-0256?áLèvª	ÀEtžý†¨üÀ:ªÏmýÀ<Ybцoñ@'{^p"Ó?ÿøŽ‡à?ˏhc?Ñã<$ôV)?ý
O#SÂ?ÿ‹çýÈ?ïõøÀ·¼¿ãí¥Ùÿ¸…äÛâ>y¿çƒ¿ÝÑ¿å(R. ý¿ïÿA^o! AGNbcuTXS 0338-030?ïð­-¹æZ?T"
«Þ?^¥¤<|\n?T"
«Þ?ïä>y@o?l±gÅT?kÁ†ã«€ã?l±gÅT?ï"/RËK?'Âb¦¬g?Šù4Ž½:?'Âb¦¬g?ï\¦bZF?tuú³…î?"k<ړï=?tuú³…î?ïæý®äQ?gÿÅ$'I´?iä…U¾È?gÿÅ$'I´?ï¤öGM$)?‡»eù~È?†Ânø…ç?‡»eù~È?îý''iN£?"ÚY‹G§? &Ö؏.Ï?"ÚY‹G§?íR¼Q³?›ss¤™P>?µo"rgã?›ss¤™P>AGN4FGL J0342.2+3858?Ä:™)ÃYÀ)˜øçÝÊKÀ:QÝIÒÄÀ<9à+Nbd@9ºZ.t³@üº€™îS?¾–y(µÖ¼?–Úâ}ýˌ?Õý†þâHµ@NžT¿J?íó
¾¯}²¿æ4M¯¶;'¿å¼ùðòF¿âˆ^Þ²¨¿âÞsV–¿ëšŽ ¿"(AGNfsrq3FGL J0342.2+3857GB6 J0342+3858?ïþùs…?ªalU? hÆäGR?ªalU?ïö,düž?T/'§­?RŦؑe?T/'§­?ïùŸÁÚ^?8.ùO-Ô?I€øµQŽ?8.ùO-Ô?ïÿ™€o&)>öÒhV`½?	Ÿô¢þ-m>öÒhV`½?ïÿ4¼Rß©?N®fQ°?hnðK›?N®fQ°?ïҐœ""†?ƒ¼Ÿ¸T‹A?v·²
3¨?ƒ¼Ÿ¸T‹A?ïøœ0D7à?e~5«)¯<?M>ˆßTâ?e~5«)¯<?ïÿMR¹©??]®ÚÄ?UÅù!>Ð??]®ÚÄAGN4FGL J0342.8-3007¿ÄõÑË0·ÐÀJ>U⊤3À;\ù1¯¥uÀ<è~ ïÏ0@|ØãÀ¯?øï»åüj?Ý儠¹?ãJB¾ìdm@ l‡י@Úën"d¿á²ý¸ýâï?ïÜ¢ÍõÁ¹¿Ô—€DY¿×Aß3ÞL¿ìŸ_¬8¿ïòÛßå-lAGNbcu3FGL J0342.6-3006PKS 0340-302?ïáâdIè?jhòñóL'?nÿ·2ø?jhòñóL'?ïåö˜Ö¯?oòn÷Im?já	MIy?oòn÷Im?îÉ%Âÿç?­©"Y0?£m£Ðñ"?­©"Y0?ï~Þ+ç0ô?sVß@0"?$:ˆAKˆ?sVß@0"?ï‡]ÃïGe?"Øe²6s…?Ž(.&É?"Øe²6s…?ï•Åg†U?'§$÷¥ ]?ŠºÎ¬ý¢Î?'§$÷¥ ]?í挌k‰? è:ǔ88?°ËŸ».°;? è:ǔ88?/Â÷r?—¾Á¦ék?§ô}<Óá?—¾Á¦ékAGN4FGL J0343.2-2529?ên*æ±OÀIÓ|ÌyÀ9ÊdpÂà»À<d‰éù-~@Pm"½¿i@±oɼw?·*Aë1è?Âo'Ÿaµ@¡âއ	t@ҏe?Ô‰[l¿ä\¦(ô¿æ߆ôÛ	¿èq¼Û¾¿í2ê£whí¿ïüwIãxáAGNfsrq3FGL J0343.2-2534PKS 0341-256?ïýMRÍ?)4—žÜo?5— ¼£Ð?)4—žÜo?ï÷Z(/–?R)G?»G
?QKóñ™RÔ?R)G?»G
?ïå›ÒGϼ?VV;ð?jd-"|?VV;ð?ïþØù‰vê?¤‡'4­‡?"pdø'ê?¤‡'4­‡?ïùÝ{"¾?B8ÎЇ!ò?HŠ(´P?B8ÎЇ!ò?ïÙÉjA½:?v8À\BHi?sJü®þ?v8À\BHi?ï³ÂèÐìö?{3–4?ƒEÀ«?{3–4?ïüéMiÜ?0ìñ0ô?8µ"éÛ4j?0ìñ0ôAGN4FGL J0343.2-6444¿íÈBYÊTUÀEÔa¿7¸ÔÀ9y'S+ ?À<Sá,Ö"@ýt»¾³@	…º¿"?¬IƝˆ¼}?§áUšç!?û'YY7©º@Çl½Ãp?ï ±ád"¿È™òD€"¿äCN¾ÿږ¿à`)k3TÁ¿çí¸4Sſײßð–AGNbll3FGL J0343.3-6443PMN J0343-6442?ïÿ½¸ª"?nJ¦ÔÈb?ÈG$g?nJ¦ÔÈb?ï÷a0¥?U%óñàÈ?Q=ž—•ht?U%óñàÈ?ïóڙOX?_Ù*Âæö?XJÍâ)?_Ù*Âæö?ïþ&'d@ò? 7¬Kñ<?-–ë"a´? 7¬Kñ<?ïþüá×9Ò?À‰ýÚíN? 1ÞPDŒÍ?À‰ýÚíN?ïÝ;ÐÍS?râ¦íƒëK?qbß\&à?râ¦íƒëK?ïîASÝLÍ?mž±®PÇV?a¾¬KV?mž±®PÇV?ïüü·:I?0V¹ª+?8D]í"?0V¹ª+AGN4FGL J0343.4+3621?ì§þ4+‰NÀ-fãOÆñÀ9ð¿§J\EÀ<jÃQ#@®Uÿfþ@€W$'°?ĘvßE?ÃÕYä!þ?ý&¾æZ<Œ?ÿe*ß|¨¿Ð"á+~‰¿é¹vCS;ç¿ÖÄO»)6Z¿çqÿ Üï¿ç
J5®7¶¿ïëa½µ,ÈAGNfsrq3FGL J0343.3+3622OE 367?ïèÒ/kÜ?eȚՃ&?g-ó®86?eȚՃ&?ïáò:'î¢?j»Òuò?n
Ş+åç?j»Òuò?ï™.ÖŹ?ƒ9/\ZÄ?‰´z|!à?ƒ9/\ZÄ?ïVïr`'?vU'ÓoZ?•"ºÌöç?vU'ÓoZ?ïPsËSÐã?'0!}J¥ã?•ñ†—=±­?'0!}J¥ã?ïZ˜¡ïJó?™éŸPÂÚ?"¬ëÇ>Œ?™éŸPÂÚ?í=Ɋß'Ô?©ºA¼°As?¶³ª¾Z?©ºA¼°As?ì_Õ0Q4?£õP'§ƒ?¿V}v_?£õP'§ƒAGN4FGL J0344.2+3203c¿î¢­ËšÀ1ìP½‡µlÀ9q±6nQÀ;5º‹¨â@ÿúPh£-@qÅìÞ»?בÁŠúD?Ý×°UÁG@"˜Ã°ÄY?þÎõü›ò?陊€!"¿¿T³.@/¿è«ÆÑá	¿ë!jÃQ#¿á0–5a
Ý¿ïí%g˜•ŽAGNbcu1RXS J034418.2+320903?ëô"ã$[?ÁôIs;‹ò?À-¬sïn–?ÁôIs;‹ò?Ø×ú"ë•÷?ÍP¦‰t»ò?ã"¶
5?ÍP¦‰t»ò?èÅûÆE°J?±Ð>x4?Ìèæé>Ú?±Ð>x4?Ø¡¼I-+Ã?¶·RÊϲà?ã¯!Ûij?¶·RÊϲà?æ54?LÇ?ÑË¢¼i9?Òý•—fr?ÑË¢¼i9?¸Y
|>?¿77µàx?ìÿ_Tµu)?¿77µàx?á¹Y;õ=s?¼Ú* ˜"y?܍Mˆ…?¼Ú* ˜"y?‡ÊÙFq˜8?€—àɑS"?ï Ôšæ9Ÿ?€—àɑS"0MIXED4FGL J0344.4+3432¿Î&Vš°4À/ô‡B_À:ÿ@ÿ¤À<ï< @!v_[…6á?üÊÙþ
·y?ƎDÑÁ(T?ª‡1j…@?å‡q^-O@WDŽ¥J¿ïö«!ÃI?ì{Ϲçû?È6â?OÌ¿ÐÑLŽNý¿æ¼Áò~7>¿²PÂæ$AGNbcu1RXS J034424.5+343016?ïþÿpIOe?>perÎ@? ý¨û˜%?>perÎ@?ïô´ìËÁ?WéÃpŠ.%?V–&«æý=?WéÃpŠ.%?ïò|ÚF2?cœ&·?[K—WÈÝ?cœ&·?ïíÜ[1?K¬ˆ'…9
?b<d¡?K¬ˆ'…9
?ïý§-RQ?2Gý¸§Çí?2ǀ[-¸?2Gý¸§Çí?ïÏ`\Ùl:?Ø(´æ/?xOÑ£Èû?Ø(´æ/?ïíÏ(;é?u(ð{õ?b0×ÆHvÙ?u(ð{õ?ïÍ£L~fk?mªÂ6Ÿçû?y.Yº~?mªÂ6ŸçûAGN4FGL J0345.2-2353¿ÅÑc=ÄÀIj³=¯øÀ9@ßìdAÉÀ<Dªùš‹@ƒ°f·š@G÷`MÉ?ªÐÌ`Á5ë?²¿ïn¸D€@P<Íæ¨@	n£Rÿ•¿×˜ÑÞ«Ü¿â™ð‡Ôö¿ç¦]¨R¿åˆGä¿äÑTá®±.¿ïÿù_|è3AGNbll3FGL J0345.1-2353NVSS J034518-235218?ïþ•©
ïœ?òæÏ·ß?&¥kn?òæÏ·ß?ïöÄYœæ?R±J´ú?SÞw4	?R±J´ú?ïðwR¿7?i'ħw›H?_×쎐?i'ħw›H?ïí´ÑƒjÙ?OéDº¿j×?bK.'fÀ?OéDº¿j×?ïþž°H¡s?™Ä)Yë?&÷ãZ?™Ä)Yë?ïÓ!€nÅ?€–j×掛?vo@e<?€–j×掛?ïíñ¨¬å"?i|pÛ»Ï?bWfXK‰?i|pÛ»Ï?ï§å1‹?y'æŽÉ?†ÀÂq<?y'æŽÉAGN4FGL J0345.5-3301?ïD­. ûÀJeè'%À;(*FûgÀ<ÇMé—Þ®@åכ‡Û@lCõù?ÆÐ=…³:¿'ÈZ]É?Êá|œ³ªg?þ|jvìEŽ?ïÇ@f!¿è¢®Á¿ãq•+uпæ£Þ+™á¾¿ÙòÑäcÂG¿ïó²I"ÇÉAGNbcuPKS 0343-330?ïüôE?Wâ?(t1bž?8]Ö@ "Ö?(t1bž?ïõŒë¾Þ?Xñ	Æñ?UÀåÈM4‡?Xñ	Æñ?ïæP-·?¿?Vì'óŽÖ¾?i¯Ò5?Vì'óŽÖ¾?ïøñ*ŒŠ?2–möø?L9ŠNx"á?2–möø?ïú-íñW?Aq_)j>5?GHG'x¨L?Aq_)j>5?ïÒbÔÇ©3?'àsž¹c?vŌ]2Ã?'àsž¹c?ïÍ¿iɤ?z}gÑ8?y K2,Þ?z}gÑ8?ïÚÙëCZs?bý'l¢¶;?r"
MÔ¦¸?bý'l¢¶;AGN4FGL J0347.0+4844?똅â'Àg|¯Ý©À:tü+_)À;¥ðFN™@²Æo­G@©âå=?É?:èß'?Åu°†E)?ù´…xze!@Í~¦#?Ë?æm®YD>ô¿çnµŠè¿åK—"pî*¿ç—IBi1¿éöÒÅ4R¿ïþ YQUAGNfsrqIVS B0343+485?ï÷ç·M£f?HU9ʱ.^?P0'XZœ?HU9ʱ.^?ïëµÿ'Ó?l§H–¸7?dJ#i-??l§H–¸7?ïÓ»Ã(øá?j&ä³ß?v"l3{I?j&ä³ß?ïß´¾c'˜?P#t¥AÔ?p% Ø»"?P#t¥AÔ?ïä‹ÆOã¡?i*Ý"¬9œ?kt9 þi?i*Ý"¬9œ?ï")Ûp©‹?˜\Ûé™bò?‹5‰†É9?˜\Ûé™bò?Ýïà?›/GãÕó?¥6?M?›/GãÕó?ï6S˜GN?äÙnôã?™=5†ÞM?äÙnôãAGN4FGL J0347.7-3616?窅ZzþWÀIÞÿ´€¦À:Жï›-îÀ<¶¤À>I@ý"õ•Ä@"÷H¡Y?ÇàV
??¯¬3á?0Ô?á|tŤº@¼dkd}¿åÎÃ|Áò~¿áŽ®žä\6¿â÷®aÐ*¿å°B½ê±º¿ä•^Pp¿ïÿð ¼x—AGNbcuPKS 0346-364?ïÿjÉ'?5s! >Ø?¦ß&î­\?5s! >Ø?ïø* îjµ?PËÞNK/Þ?OW{iT´$?PËÞNK/Þ?ïôˆ¶×º?P½ÔºiŒM?VïÌ܈Ý?P½ÔºiŒM?ïÿÝëÙŽ>àYÄdsQ>ñ
'Lpå>àYÄdsQ?ïÿ®L•@*?Ôèà™ÑÄ?lڗT'ª?Ôèà™ÑÄ?ïÛú®óë?t(d´EÔ?rÿÇr†5?t(d´EÔ?ïðÿ#-£õ?jï'
¹?^¹.…‡'?jï'
¹?ïÿ´XaÀå>ûÓ½˜b¾?éÛØNõx>ûÓ½˜b¾AGN4FGL J0348.2+6035?´³ Ž£@?Fí$[)À:""W:yÀ<H§+R""@!ú»+Ìw?øê`üšò?Ë!¼•?ÈIÕ·3‡?ö
ˆºNE?ü%1uBø"¿Õq7eGœ¿çåaHÌ"¿ë¡h?¯mk¿±"ùF¨Zý¿¾‹$ƒB¿ãēBgƒAGNbcu3FGL J0348.4+6039NVSS J034819+603509?ïönzö°?N…v1Ýþ~?S#	Ÿ-Ë?N…v1Ýþ~?ïßLGp?y,ñïÖÆ?pwYçöž€?y,ñïÖÆ?ïÉ£"~³ ?y	ù I?{.6<†§Ò?y	ù I?ïêIÉ2õ‡?P%ØRµÀ¹?e¶6–¹f?P%ØRµÀ¹?ïàdËûU?qË+Ì/mª?o›4Þê³?qË+Ì/mª?îß!Èœ¹?©í·Ÿ¨é?¢
ã{6˜s?©í·Ÿ¨é?ïR\dãb?"	¥¿<Ž?•¼Toó÷Â?"	¥¿<Ž?ï|'FWìë?'W^†'×?m·;᚟?'W^†'×AGN4FGL J0348.5-2749¿µóª|jߝÀIv†œfÓtÀ8!ײÙÜÀ;¤ÖO,þ@ž4ge¿Í@³¯Yõ>Ü?™9Æö*?°(U3¹
@ÂܱF^‰@ qÛ	¦qï?ۜÞ]	¿Ý s]Dԛ¿ãÏwÁ¶™¿âOðِ¿çs4_Ù'¿ãUOwÅAGNfsrq3FGL J0348.6-2748PKS 0346-27?ïý	Df%=?3Áª?òüš?7µÞòd£Û?3Áª?òüš?ï÷‹vÄ?PĞA×`Y?Qæéæx?PĞA×`Y?ïì6˜‡:?caÜ:½ú?cðɅµV"?caÜ:½ú?ïÿúüàæµ>¼…*Yôù>Ä"…|ü>¼…*Yôù?ïþτ?ÈË?!^E¶?#»µ=W?!^E¶?ïÜXºÍÇ?t}Âéîˆ?qÓ·½fw?t}Âéîˆ?ïí،¸N?tÅÈz|y?b'sj
˜x?tÅÈz|y?ïÿû™¥\>ÂGJèl…†>Á˜'^Vš>ÂGJèl…†AGN4FGL J0348.6-1609?ïÿÌeÁbÀGÐqÞi­CÀ9˜®Eù•À<Lso"
@V0S.ü@¥M–Ãü?² Êzâõ-?¯²1k

?úÆ`¼Ù9Ã@…‹TÝR?ïÿµ¿â'ºí§7è¿æ¬êÿ½ºá¿åО~蝿Þ5xó0䤿ïÿãåîAGNbll3FGL J0348.7-1606PKS 0346-163?ïþ†Äi¯?ÄF¼¿)?'ž"|¼=P?ÄF¼¿)?ï÷xä\$]?O©®›­Ê?Q7<¸†/?O©®›­Ê?ïï:¬h?fTT'äÜ?`ùþž×ø?fTT'äÜ?ïú]ǹñ?2»RD`µ½?Fˆâƞ­?2»RD`µ½?ïþ´3jV?x…×ÎáX?$¼Ê0VM?x…×ÎáX?ïØÝ+¿¡k?v"œI.•?s'j3mV?v"œI.•?ïáQßÏ;›?q²@GVui?n® 2$=k?q²@GVui?ïîîDþQ?R"*æø5ö?aᵂOp?R"*æø5öAGN4FGL J0348.8-0828¿ìŸ5Õ¿ÀFU•:À;ážëèòÀ<Œb¥Æ!@·ÉI	´4@Í6´ÇóI?̲fnžï¿qÁŒ/U‰?©}GÔUd@Ã3ºÂ‰'¿Ê¤©;¿ê'Âó/7%¿ÁüA""´…¿â=OG"=¿ë&Ü"U?x¿ïý—"ãwAGNbcuAT20G J034845-082422?ï÷NÁ?û?J͸ž,Qs?Qb~lòè"?J͸ž,Qs?ïöJQ\ê?VD$ê"Ê?Sïk?	œ^?VD$ê"Ê?ïV"݋È?†ÔÉÿ©Á?Œªw7o?†ÔÉÿ©Á?ïôe!©?>òÃ4Ù¦?WñÇ*½î	?>òÃ4Ù¦?ïôˆZ´?QY`šÒ°8?VïÄn½v?QY`šÒ°8?ïÖ(ôž€'?wm›ý2®q?t노þÇ?wm›ý2®q?ï"×€¸Á?Š`!ù†—?ŠÊߞ•?Š`!ù†—?ïÍÖPÚ
?hH~ք8?yu"÷ßM@?hH~ք8AGN4FGL J0348.8+4610?Ñxjfóv|À¨¬\ý
À:Œ|¦CÌÀ;ã¦êºô]@7Â4moð@SÍÝnÀ?Ü»"¿e=?çcÖ>»@
"x'@	õ¢š¿ß!Ã~ðK¿Üò{}Nà8¿é‹?äœw¿îÂˌZ춿ïΌŠ½]Ä¿ïÿþˆ0»ŠAGNbcuB3 0345+460?ïN·uD1?¯µ\ït`ˆ?–)W|yß?¯µ\ït`ˆ?î'1@>ß?°ÆAØO}e?®–ìïk®?°ÆAØO}e?íi~Z	G?£N_JȎ?·œ´wçÊ?£N_JȎ?í^=˜;ö{?š=¿™¬¢?µ?Ø#?š=¿™¬¢?î¹ÕÖ®{?®ß
ÿãs¯?¤b¢˜ŽO?®ß
ÿãs¯?ãâ 9¨?ÔdØb¾Lh?Ø;¿Œ{°?ÔdØb¾Lh?ç6*¿^U?µ>¢1€œ?ѓªÉCU?µ>¢1€œ?ÕJóV¬è‰?¹ d)+d¶?åZ†T©‹»?¹ d)+d¶MIXED4FGL J0348.9-4859?îïڈC¨CÀHÌM©>êÀ;i%ö3ÎdÀ<Ù=x0"F@£Zì4Ç@«ôz¿Ö?ÁýHëC¿µ¡ÙÀ6wœ?óÙ¤ì³òá@6ìÕ*ê9?ïF®€žÐ¿âH†`Կꟴeͺ3¿ØÜ̉°îJ¿ï÷b|×Â?ïÖäH•AGNbcuPKS 0347-491?ïõºv«6?Küô/r8ç?T‹ýŽ[ƒü?Küô/r8ç?ïóî
S'?[Ÿ‡†(?X#å€T{'?[Ÿ‡†(?ïśÉ'Yi?x¶¦ýP¿]?}2lSK"?x¶¦ýP¿]?ïøéߓ_)?9BŸá0â¡?LX€²àm	?9BŸá0â¡?ïÊã£vµ?zTËOôZí?zŽ.}S)S?zTËOôZí?ïʋ³
DG?€öà•$?zº&œì@?€öà•$?ïÑ2|vj?|£%¦Y"â?wfÁå
d?|£%¦Y"â?ï¹MAã`s?vmU¹ˆ?¬¯‹÷W(?vmU¹ˆAGN4FGL J0349.4-1159?äŒhv¿'•ÀFÚ$5inYÀ:E†ö(æ©À<R°«#@ öODú?úUPÊï$?Ãþ>ß¹¹u?°'_~ØÕ?ìRjÑ/2@8®©K=k?Ÿd³dÆÔ¿ç\ðû¿åü½€S¢?ÈS™Z.Ÿ¦¿àuïÛŎ¿ÜìCŠ™AGNbll3FGL J0349.2-11581ES 0347-121?ïþ‰æHHï?wóž¯÷]?'a›OvÊ?wóž¯÷]?ï÷<ºp?Q²Ð†p?Qï†ùá?Q²Ð†p?ïù¡º'ûÑ?TÁ3­©¶e?IyFW°=?TÁ3­©¶e?ïûÓþø̎?'
‡'ÑIÑ?@°çCC?'
‡'ÑIÑ?ïþ¾ó}ª?Å[vyҔ?$ÄúGm}?Å[vyҔ?ïÙU™ÜØ?tï§ä|>/?suÕ0Qä?tï§ä|>/?ïü.Ôÿ¡5?QR'Žz(¨?>‰Y‹æO?QR'Žz(¨?ïõ+&Z˜ä?ErèC—T†?U©³qI×Ú?ErèC—T†AGN4FGL J0349.6+2410¿ëÜbTf'9À7°³''dÀ:·ÔÌuŽøÀ<8.Ýc@°ŸÑ—ö@Þê· ?ÒBh$¬‡³?ÜV܅§tN@KŒ@Ã@	ޖMß²¿äïÍug‹¿ÞÓ0~¢ó5¿ëÙúnƇ¿æ‰Éb4'¥¿ð?ïÿæj,ĄAGNbcuTXS 0346+241?ïðKðV?mµk²'«
?_h Bp3?mµk²'«
?ïìúZµ¿P?dïc™S?c¥:ok?dïc™S?îT¯*H?-•>´ÿM?ªµ£±§?-•>´ÿM?ïà#›»ˆ?Y¥šþ!oC?oýÜO¦ÐG?Y¥šþ!oC?ïöåñ{?aW hƒ3?Rßî
¡jª?aW hƒ3?ï	›ñ…
?¯xzI¤/?žÞ,ƒ‡,±?¯xzI¤/?î/ߎy? T/|üG<?­Â`¡‡? T/|üG<?íh$Ñ	Œ5?¥5uþ¹ù?´¾ÙwEªÜ?¥5uþ¹ùAGN4FGL J0349.8-2103?æØ£÷…KôÀH"tûTŸ•À9€'،À<·ÀÌ
Š@ÐÃAØ@¶øº'`æ?«Û®¢Ñ?ƪ[É)*@Aél?Ä;@w¢jxš?ºËŐÃ\6¿âûMÿm'¿æÊé½ôAÜ¿èÂ:ØC""¿ìd3áƒé¿ïü³µ¥iAGNfsrq3FGL J0349.9-2102PKS 0347-211?ïá4"úßb?mͧ½ožá?nËÜÒFeí?mͧ½ožá?ïôVÉ1Ú?Xs¥\";?WRm1Q?Xs¥\";?îãpÙÿ2?—ŒK`"?ö?¡ÏˆïÌWç?—ŒK`"?ö?ïú²ò
׍?2Ëj­ÿa?E47çk?2Ëj­ÿa?ï½ÓÕՊ?~çŽéÃË?€‹
…Î	[?~çŽéÃË?ïÓCñ"Íõ?wÂè<}Öc?v^%šå?wÂè<}Öc?îŸ%2¥ªÛ?ø¨‰%Ìü?¦
¬Ò5¶S?ø¨‰%Ìü?ïäJÁ´Â?\eÖ€ZÈ?kµ>0^6?\eÖ€ZÈAGN4FGL J0350.0+0640?éIèº0ÀA"ãÞaIÇÀ;…BêÊÀ<–'nQí3@#Ç£Œa¢²?ùN"wÉe9?ΝñµaÌ?aoyyWsž?ž]÷íÛÕ?ý—ÁREG¿îb,°b2û¿*Ù>ís¿éTr]•‡f¿Ð$÷0M¦¿ÕÝìd—¯4?Á].Cà)¡AGNbcuNVSS J034957+064126?ïÿ-­7[6?_"eÿ"}?JR,•{õ?_"eÿ"}?ïö?ÙJ?S9.ŸF
?S€Mvx?S9.ŸF
?ïïû°1'ü?PM6_aBÙ?`PvÃs?PM6_aBÙ?ïû«§¹
?1l=Ha'?AQ`k·Ëi?1l=Ha'?ïþÿÕÁE¹?É® K%? ¥,³'.?É® K%?ïÖ³	τ?t-¹™
Ê×?t¦zø¡–X?t-¹™
Ê×?ïï®õ)?gÙ#·³½?`Q&Oý?gÙ#·³½?ïáô…^µS?j!ºÆ?nz³(¤£?j!ºÆAGN4FGL J0350.4-5144¿á=B‹j׺ÀHDââ¸Ç\À;ªœ÷,À<Ç÷øʂ@ Éh»€I<?üªzýÍÙ?Ã:h[´×?ªà#Á¦(?èÛB±Ux@žÞýÑÒp¿îÔ;kç?àÖD°39¿ã&…¥ÆΆ¿Ð¦c"¥¿Ü¤ßÈÒí¿Ú'Z›WûAGNbcu1RXS J035037.0-514457?ïÿ@ÛpV?±êvO߀?ä"îíü?±êvO߀?ï÷-o5(<?P:ìJØQ~?Q¥"!'?P:ìJØQ~?ïöÑ~ÉoÜ?Uݟý9¾?R]ÒÔ¶ï?Uݟý9¾?ïý
7«,? y.Þóg'?7g°P7«;? y.Þóg'?ïÿ0/PX;?æj–u?ú¶žÂµ?æj–u?ïÙùÇ	q÷?~ŝƉm¦?sˆUˆJ?~ŝƉm¦?ïû> m™?Vlþ?:oi?C€+g²é?Vlþ?:oi?ïõ®ì£=?F±9½è÷?T¢';€E?F±9½è÷AGN4FGL J0350.6-3226?êìî‡K}ÀI"ìé¢ÆiÀ;ØÚø»À<ÆEéïƒ@½Õ
8!Ú@ÀRP.ì}?ÑHµüPÈð?Ï¢$Ø|ƒ?ö!‹»Š…*@3I!ßÏ?ï­¾Ña‡¿Ø؄{zIÈ¿ã<6¢(‰a¿å
pᔅ¿çב#'¿ðAGNbcuPKS 0348-326?ïýúÿåþÍ?&³Ä¥?0'ÿÿ!YQ?&³Ä¥?ï÷[‹cmZ?Tž"ÒB›œ?QHé{Ëu?Tž"ÒB›œ?ïКœÎØ@?qZ
ó¿—?w²±{·(D?qZ
ó¿—?ïÿvüœÚR>üLê›UÉw? m(÷@>üLê›UÉw?ïÿp-î…?ήÌd?ú;Øù?ήÌd?ïß-çò?saRÈub?p}ésüC?saRÈub?ïª{U«?…¦/j€ñ:?…a±twc?…¦/j€ñ:?ïÿâ
Àw?3Î6é>k?¹
‰¯?3Î6é>kAGN4FGL J0350.8-2814?äŽYW'Á—ÀI@Ü­¡À;;y‹YÀ<¤v¾£>^@"ÒB?úkKøüր?Ëv5{âÏn?¨g=beø?ßUŽ7ï@;­$æ¿<¿ïÿm¾Ÿb†?î½µ7"Ñ‹?É®«d_1¿èÀO`c?Ñt¬¥:¿¿ãÎ#¯1±SAGNbll3FGL J0351.0-2816GALEXASC J035051.31-281633.0?ïÿéÞD?7f'k9Ø??Šèä¤?7f'k9Ø?ïö€4˜¸ô?Tìôû4'?Rÿ–ÖÍ'û?Tìôû4'?ïâ0¶Ÿ ?pV…âqh'?mÏþ/CX%?pV…âqh'?ïþ>± æ?!)ãÉ&›¾?,U.'öW?!)ãÉ&›¾?ïþÖ׊€? ÞOc?"'…éb~€? ÞOc?ïÚ3g=?u•$åš?rær¬Å\?u•$åš?ïÛûNŠü?wξóÿïJ?rXå<aÝ?wξóÿïJ?ïú7Î<R?C†–§2Ê?G›!0'Ñ?C†–§2ÊAGN4FGL J0352.0-2516?âõ·^wÀHÕ³co;!À;R>{fÀ<Å憲6I@}pŠìÙ@"Pi¤ßH?Ó°°!á?·óÔMŸ›?䦸ÁRT@fA'šÇ—?âd"¿éöñL¿çÛBEÈa¿Ïˆâ|·`ª¿èàYTÔ¿ïúÅÞÆõGAGNbcuTXS 0350-253?ïû€7a?9ží¹|óü?C­þÿò?9ží¹|óü?ïóܯN?Z99g?XF¡o¾ä3?Z99g?ïÜ_ÃEJÉ?p˳åý¢¼?qÐPü‹?p˳åý¢¼?ïôMís¶[?<€p¶,¦$?Wd%GMùˆ?<€p¶,¦$?ïû=U~•?8ۋźù\?B
>Eá?8ۋźù\?ïÖÀ(Î?u$Íà`6þ?tøáį?u$Íà`6þ?ïÉ8äU³?€kQØÈØ?{cèdC©?€kQØÈØ?ïÁê!,± ?l[¿³"›z?
ïLÊx%?l[¿³"›zAGN4FGL J0352.9-3623?ê¼3Ô\§åÀIYJôðØEÀ:øº˜â›À<uä;~[P@!@iGA]?ôÜZ>9÷s?Ê^Í?äF'?Ó7þ(Š@	™N?Fg@µt«ùm•¿í·4µs¿ë¼=¾&–Ã?æC¼ª R¿Õ‰Ïa§Ñ¿³`#%¿âh'Ü\AGNbll3FGL J0353.0-3622XRS J0353-3623?ïøSÜ &ç?Iƒ¨'³uK?N°™ÇÊo?Iƒ¨'³uK?ïö>äÓdþ?R¬TM/kÒ?S'6¾%6?R¬TM/kÒ?ïÏæ\jå?sðM•=.?xw±~9¯?sðM•=.?ïù¤üE­¬?;R£÷Z?Il÷Ä)Ç?;R£÷Z?ïøšDÍv?Nu©ajŒ?M—Çv:ˆ¬?Nu©ajŒ?ï×bAé"i?wå=
Qú*?tNß#úû›?wå=
Qú*?ï¢7|»^Þ?ŠEœ?±ÞÄ?‡r Þ渃?ŠEœ?±ÞÄ?ïëJµ›¶?^†eOß?dµälÀas?^†eOßAGN4FGL J0353.0+5654?Ï0竗ÀH@¸ÌŸóPÀ:ÚH¶RÀ<VÅßrÂ@ jÞ~¥øM@CÂb¿'?ÀŸR–$ïù?µ´"K æ?ó5'éSì@ŒS'Þí¿ëo>&VV?ïå…?ðZñ¿Ø½ây1o¿ß,'Ûç¿ä'è̱¿ä61_žv"AGNbll3FGL J0352.9+5655GB6 J0353+5654?ïýúÏñ?"ßWhB›È?0)ˆ'R¹?"ßWhB›È?ïê7"ÎXŠ?t0ØiÕÝö?eÈÝ?eåp?t0ØiÕÝö?ïõ½Ä¶]?V'ÉYxä?T"xYäx?V'ÉYxä?ïöގ–0?;¹DB'û"?SÔB"¯¾?;¹DB'û"?ïý|Ó\?)Ÿ†ß™N?4gZ=Ýô?)Ÿ†ß™N?ï¶‡…g?¬0u;0ü¤?ži>ò~ï?¬0u;0ü¤?ïïḨcÈ?må|<'ºt?`GR×û?må|<'ºt?ïãHÀâÉ?\k
8á‡?l·?Ëà§??\k
8á‡AGN4FGL J0353.0-6831?ïôáªÅÀDbŒL˜_À:r)ñkÀ<qä"rÁ@!ñnmpñ°?ú.kßL+?¾n­¡},•?›¹·Ç,#õ?àáP¢"ϳ@ó͞Xñ?ïT{昿Ú{´Á¾%ë¿â'OÐø«x¿ÑĪ¿[Ë¿Øše¼Tº?•©˜5ÁXAGNbll3FGL J0353.0-6831PKS 0352-686?ïý!ŒJYH?%Øöé.#?6ó9Â߅?%Øöé.#?ïôà˜—Í"?Z¬¦ÃÎùY?V>Ιküq?Z¬¦ÃÎùY?ïòŸ—[?\É7͑å»?ZÀÒ:ni¬?\É7͑å»?ïö‹왭?<#ˆí.wF?RéðE	5ê?<#ˆí.wF?ïù•\•yœ?=P
þßåÿ?Iªüs¯?=P
þßåÿ?ïÜdÎqù©?sT¯'ÓÏo?q͘ßÀ["?sT¯'ÓÏo?ïôÛ,ÈH?hƒF]Ý9?VI¥ëØoß?hƒF]Ý9?ïå>¯ÏL?Z?§£.+?jýÁq,ó"?Z?§£.+AGN4FGL J0353.7+8257¿ìÈ@">Á@6Q?´‰À;X®í¾µÀ<¿í
´ôi@!Ӑ¸ŸnE?ú"âÀ*'?Á§¦b)ë·?¨¦ÜOKÃ?éÐ_Sw¡@à[\È
¿ë"m‹?ïýä1m`V?චpMoõ?£S=ÏÕ|¿èšˆҜ?·ÊùŸ$QAGNbllWN B0343.1+8247?ïümÙø.z?@›'z:¯?<'1ûي_?@›'z:¯?ïññ¹|t?_1"DÁ‹0?]ÆSèF?_1"DÁ‹0?ïÑ8h"õ?{¤É¹Í	Á?wcÌ"½v?{¤É¹Í	Á?ïÛÑ1¶[q?^®íLE?rg>?c=?^®íLE?ïñ°§°¼)?Y	6ögg?\ž°–¯†?Y	6ögg?ïÉó9Ú'?'Üo®5 ?{c-¹,?'Üo®5 ?ï°>X5u?†½L[‹1›?ƒðiü\À?†½L[‹1›?ï·p	'q?yQLšØžë?'#ý¨eN?yQLšØžëAGN4FGL J0354.4+4643¿½ÄM¯úôÀ"¬ó±³À9,ó*.§³À;˜ìÿr;‡@@õÜ»'M@*º:#?¶` ¦Õ?¼ÃÎ!`£@§Å¬G@(BÒ¸t%?íQ5aáœh¿âY>?€Éi¿èw
bZé¿äœ¼cÈý4¿ê§l ½$c¿ðAGNbcu3FGL J0354.1+4643B3 0350+465?ïû'þÿJ?3TÇè?z?A´.ü5Y?3TÇè?z?ïï3•"ãc?h^·¨uI?`Ìj—!?h^·¨uI?ïÝuqF>S?eWi§C:d?qEGzmzq?eWi§C:d?ïî¦T¼ø?Hµ;E•åÜ?aY«õÁ'?Hµ;E•åÜ?ïø‹åÚm}?GFŠNdÿ?MÐh8Gð'?GFŠNdÿ?ï£JøªT?"T/1dߥ?‡:mEE?"T/1dߥ?ï¥öXÙ­R?ƒ·7@N­?†'iɔ«k?ƒ·7@N­?ï´)¸éž?mé[x?'õ'ÎßJ£?mé[xAGN4FGL J0354.7-1617?áÅFsàUÀG)l?Ä;.À:û|üªàêÀ<€ž @I¥Î0O(@×N›n…ð?͆-—¡?³ÓÄ[d*?áº}ibD@"hMò&N?â"õbîâ¿áuҟʋ)¿åw©Ÿ¡—¿ç‡¶"v¿ïÿ•Âû?è½hvAGNfsrqPKS 0352-164?ïÿDW·¿?–ÑÿdÅù?u_<'?–ÑÿdÅù?ï÷à­L?SçÕßä[?P>¦V0U?SçÕßä[?ïéü!ñcÒ?am8=?fÞ*
€?am8=?ïþß;M:?LªKM$?"HÛ*É©?LªKM$?ïÿ¬B5&?©S•Iօ?ïstw$A?©S•Iօ?ïߟTf1?smd@¡"?p0U±ƒk?smd@¡"?ïéȑ?rª€NöYw?fä7™"§?rª€NöYw?ïúø3$g
?6®Rb5¶&?D4i#ª?6®Rb5¶&AGN4FGL J0354.7+8009?ª'Öä3@4á?J˜«À:[í£)æÀ<–!à$˜f@vlÉ×Ïà@SR"Ã?ÀL"½ê[Ô?À¦ÿVýé?ûpû€>~Á@tP¬ñT?â­ž´5§?Öë©|Åñ¿ã"_½Õ¹¿åv·'"…¿ä»¢£-—¿ëKf/ßÁœAGNbll3FGL J0354.6+8011S5 0346+80?ïþ›HgÅ.?ºÅcµL?&KwÇyBÊ?ºÅcµL?ïôôý©Ÿ²?Z1lEåȵ?VÅ}ËL?Z1lEåȵ?ïð¥q5™·?YßÌc-ge?^µ¾áA?YßÌc-ge?ïÿ'B÷>ùü™ª­?olžÎ@€>ùü™ª­?ïýcÁ׌€?1gø¹KÚ·?4áïÍƅ€?1gø¹KÚ·?ïÌ1™!›þ?|êgÞOÇå?yç3i² Ð?|êgÞOÇå?ïމb¿½Æ?xT
«Â/?p»N´Ù?xT
«Â/?ïÿkýBû?jKà¿?€VJâÏ"?jKà¿AGN4FGL J0355.1-1841¿Ùß*¿¾"ÀGËs2'À;?¦½oÀ<ÇQâJãS@ Êæm²¶?ý6Ó¼)ç?Ñkúú݁P?À!hE
Ñ$?짧¯i?ü¨ÚiÃh¿í(¾ÐŠÇo¿ì	| ºu1¿ÃP"'5ú¹¿ÕEM\T>Ç¿ïхc¯˜?îÉ,«AGNbcuNVSS J035513-184309?ïýd€n`—?0¼·Úz?4Ûû~€oà?0¼·Úz?ïõCÿxØ?U
]Aõ¦ß?UyçèQ ¦?U
]Aõ¦ß?ï¤%""Îÿ?}òÉhð«Ž?†ö›,Š°D?}òÉhð«Ž?ïðȔ{D?P/¼ë›½?^n׊©.h?P/¼ë›½?ïý^ôhXj?2Ãì4æK'?5\8u¿?2Ãì4æK'?ïÐ9«¥é?zzNˆºÖ?wõc3V?zzNˆºÖ?ïÇ7*Iæº?…+¨AS?|djüâÅ?…+¨AS?ï®›‹m?~Vo{Í{ª?"~K۔Ÿ?~Vo{Í{ªAGN4FGL J0355.3+3909?좠-SíŠÀ&uš¶ÐÀ;gÐâÜÀ<w´ÃÁ‹P@"­e«£?ü¤
5ãè?ÐáÛý—E?¤l…~	?ÙuJÅK#??áÀÛ'£H¿ïêu¿Ÿ½ ?ïþÒn¥Ð¿ÐœEÛ×V¾¿çšãEµ¿½TfÈ{"¿àÑ(l0AGNbcuCRATES J035515+390907?ïÞ|%{ Æ?­Kö=DÀ?pÁí/¡¸â?­Kö=DÀ?ïm¨¬­Ú?œÀžxøû"?'Jÿ
jDË?œÀžxøû"?ïlIܺM?{cüñÜ?'vÄjn,?{cüñÜ?ïRùۉå-?…]ùٕö?• Ä"êÄ_?…]ùٕö?ïü0ÿ–"?E»Y"P?>x[,F?E»Y"P?ëèsñ¶³}?ÇE\ 'G?À^09%2?ÇE\ 'G?ï‡=û€?!Ý
¶?Ž0*¡?!Ý
¶?꼆ËÍ°?¶–¬GyÄÆ?Å
çðÐÉB?¶–¬GyÄÆAGN4FGL J0356.1-1329¿é`\'{hÀFq[ÕìÀ;,ÓD¶vÀ<µ}¼Ä@´HÔÛ.?ÿ<r\=îx?Ñi·¿Ža?¼nvÖ 2¥?ëw "~–@a[0RX=¿í€
Fªß<¿¶Ê=ü9÷È¿äüYòŠÌ¿×xXKo¿àKs2&Ä¿ïöÐâC6AGNbcuNVSS J035611-132908?ïÿ?½I?°Ê°"?ONÛ¦ù?°Ê°"?ï÷O!Ñ6?Q¼êËË#	?QÓbƒk?Q¼êËË#	?ïôw-³íX?\¬RÄè?W¥Øª?\¬RÄè?ïüyõSBŒ?"Íëǎ=¡?<0UzϦ?"Íëǎ=¡?ïÿ£cÇЏ?ˆ¨j+ç(?'ßWU±?ˆ¨j+ç(?ïÚ×2g—z?s²%ÝWZ?r"fÆöþ?s²%ÝWZ?ïõîäF2Œ?cñ5ú!?T"7)cXñ?cñ5ú!?ïð"j
9ú?QÄFD–¶?_»+iÚ?QÄFD–¶AGN4FGL J0357.0-4955?Þ¢O‹ÑÀH	‹`ñ²_À:˜WšÀ<žßVø4@]ÁÒî@¯!Áçã?¶Ùã`·û¯?·!ÕgÐô¥?ÿ3;C£@^ÎTsö¿é‹fe¦Ò¿Ñy‰¤*¿âÄãß»¿ã™ã€îR¿âĀÍð¹¿êv›r·®AGNbll3FGL J0357.1-4957PKS 0355-500?ïü"£O>Æ?4SÆC飳?;bã§À/ÿ?4SÆC飳?ïô…q°K?WGÅ¿!ö?VõEWšh?WGÅ¿!ö?ïåîðÚ»?q1Ŧ#€?j_Tb?q1Ŧ#€?ïëØq¬ÑÁ?M8'Ø"»?d'Ž$s]?M8'Ø"»?ïó…ˆÀƒh?V®¥©m?Xôï*~£?V®¥©m?ïÒáÆô?zf¶Gñƒ?vØÈÂs?zf¶Gñƒ?ïÄæ'ª?ƒÇ™PÛO?~=ŒÔÂk?ƒÇ™PÛO?ï˜+T‹?zPߌ?‰õ*÷Àåe?zPߌAGN4FGL J0357.2+2320?é`ûC
tVÀ6zÞÑ·À:ŒÄ¤	_$À<Legbå¨@ùþ«@ÿÉ^ƒC?Â8‰‰V*"?¨<S~"j?çسiy@ž'¯jfP?î0A`ó_ß¿ßztÛt/}¿éƒ1èEÏ¿ØӦύ¿ä¸é@ ¦¿ëL°/bAGNbcu3FGL J0357.1+2325MG3 J035721+2319?ïû68'Ò?4G Ç¥Ÿ?C'ٜ|Þ?4G Ç¥Ÿ?ïòo'EM£?Z¼Á§€¾?[ ÛՙÉ?Z¼Á§€¾?ïë•ýOC?a)gÿÙï"?djp$W²?a)gÿÙï"?ïÝ8ÖÇ]³?OgˆSâ½?qc"§OæK?OgˆSâ½?ïê¾üpÔ?`þ¥:vC_?eAé=H›\?`þ¥:vC_?ïÍ!hQðZ?€íç±KZ?yoKÖWæø?€íç±KZ?ïà4ñNab?te|Ëöj­?oË¥@!?te|Ëöj­?ïD §Ÿ?}šûm?—‹ñþD?}šûmAGN4FGL J0357.2-0319¿Æ^iž:y_ÀCÖb^™éKÀ:È5A*l»À<]IfË@!›ÖY¾bQ?ú³Qf$!G?Ç×&—ïJ{?Ã
pÖ×½—?ýÅÆHNMk@†¼
Ý©"¿ïÿ^Ê¾¿ïƒƒwï$æ?ïÿ‹Á>Ï¿á§Áåèý…¿Ó¦¶ão+¿Õ,0àr›ÿAGNbcu2MASS J03572609-0317596?ïÿcM?dKªˆÌ?³‰|I?dKªˆÌ?ïôÏj‹äû?Uª€B?ˉ?Va+igY?Uª€B?ˉ?ïô¦2.P?N°t¨à£?Wô³T+x?N°t¨à£?ïó©£å'?G–—=žü?X­Ø†º|è?G–—=žü?ïüþ*½ÃÅ?9¯§4¦<£?8¨s]ÃÓ?9¯§4¦<£?ïÔb!!&°?€êö¸K‰?uÎïc?€êö¸K‰?ïçb¼Q™??sP(»??hCÉã¡@?sP(»??ïÙ¦h'?o@¢Wd]%?sw,à_?o@¢Wd]%AGN4FGL J0357.6-4625¿âT¯¸GÀHd\6fÀ:äÜüŸÜÀ<Ò´%t@ô¦›µ¨™@³'[·¶»?"xŠ«?3?®ªc°y?ëGæ^d%@#®ýY¬?ïíZPü¿ÙúsCn"³¿ä³R"ÿÝ~¼¨š¿é"a å¿ïÝDuAGNbcuPKS 0355-465?ïûåzSêI?3'mfg5º?@jÊ-…?3'mfg5º?ïööâÞ?TM«EÒi?SðœAÄ
?TM«EÒi?ïè<ŒUí?\‹žòÝwQ?gñÃoŠ‹7?\‹žòÝwQ?ïòCƒ¯ÄÌ?A'íS|o?[xø‡¹8ñ?A'íS|o?ïî¦4÷Gd?VÌSš¤¹
?aYË1óìA?VÌSš¤¹
?ïÛ20²X
?rVbG}Ùÿ?rfç¥t"ý?rVbG}Ùÿ?ïÁ…Ù@?€–üÙÃ?8ÐQ0?€–üÙÃ?ïÐbç^|?cQç»%"?wΌjÞýp?cQç»%"AGN4FGL J0358.0-6946?ÜÈêŒr·ÀCÛá2µ^òÀ<'³1fªÀ=Šlê&3@˜<%u/'@|x £?Ý}Œó˜ép?ï>ž¦Ÿ@ÍýAÞÌ@…*ÁõƒO¿êÝSb}£š¿Ûí¼[t'?–"MWÕ1©¿ã³_¿-R¿ïüz¿ï—7z>ŠAGNbcu3FGL J0356.3-6948PMN J0357-6948?ïƒ_å)?'b4õÍn??»rU‰ª?'b4õÍn?ï*<ÃËá?¡n²6Ù:?š¸mêöÛ?¡n²6Ù:?ìÛÐ~ï0?¢Ëö'ØïÂ?¹'¡z¾¬?¢Ëö'ØïÂ?ì[	šÖ¢?¢·ºxÙ§ô?½'³/9Jò?¢·ºxÙ§ô?í¹¶`Šëg?¶Vm³??²2LýÎfD?¶Vm³??량jð?Ç¢ˆ@*èa?ñÚWœA?Ç¢ˆ@*èa?è ÷	Èfó?µ#ݖ"à?Ï|#ØÞd5?µ#ݖ"à?à÷¸*JÏ?ÀŸGû¹–±?ßЏ«jc?ÀŸGû¹–±AGN4FGL J0358.1-5954¿Û	U`§ÀF=žbV6mÀ:ëIBi1À<Ïs]Å­õ@oéò¢t@¿Š:›?Éç<t$•?ÁŒwG4G?ñíÏ`ûÃZ@oûe'?ïýfȋõl¿åÍEbàŸè¿â˓¿å­÷¯î¿ëÒEb	àT¿ïÿôw5ÁƒAGNbllAT20G J035814-595233?ïóëåõEo?UUer®?X(3Ë='j?UUer®?ïóMGº?Y£Îêqíë?Yep>ûÂ?Y£Îêqíë?ï§Û¸fÓ
?~"`êw?†	Ûühç?~"`êw?ïß]«µY?TOù€Ÿ£¥?pQ1‹©?TOù€Ÿ£¥?ïÐ(W%ð?z/'ÎÔ?wükÐMÏ?z/'ÎÔ?ïÍÆOºq?'8ÀxC?yØBÁ¯"?'8ÀxC?ïsæ‡"?.#oiñë?'ƒ/üo}?.#oiñë?ïxÁÊ\§m?w÷*£è?çƲ³D[?w÷*£èAGN4FGL J0358.6+0634?ÝÆ]'+À@Èك"t—À:6
fðÏáÀ<
$ÜX[@ê+‹p@¨÷ÛnP?Ç.ìË?É1‹þ¦c¬@¯/:€.@‰!.-?åkì O+¿Ó9€TN6¿é°"òsP¿âü^pпïÿþˆ0»Š?ïòF~"…‰AGNbcu3FGL J0358.7+0633PMN J0358+0629?ïè¥"Ñç?i%—p[¾?gZëIàº?i%—p[¾?ïöcˆ‰b?U͝%
¢?S9֑wÜ7?U͝%
¢?ïž_ØòcÏ?€3!2/H1?ˆh	¹8Q?€3!2/H1?ïû«çTÒ?+¶¾ÄË?ASôZúd?+¶¾ÄË?ïÚv€åÔ?v?¶4?rÄ¿ªªÙø?v?¶4?ïـçh{â?t‹Xü®?s?ŒN¿?t‹Xü®?îy²™ìæ?›2^»»ò#?¨dÖna1ž?›2^»»ò#?ïæ Vì~?Yñœ&r¿?ißç"uÙ¦?Yñœ&r¿AGN4FGL J0358.7+7649?àuxþwu@1Å÷@=ݱÀ:ɬQ,B~À<¡ ÔƖ@c/p0?ýÑÍ¢µ¢?Êm®Ú˜A?Òc¢ýe?þÆIàô¡þ?ïv%5;¦¿éÔMdº¿â£˜@S,M¿Í5AU_ØÙ¿â-sk1§B¿ê:êýdo@¿á—}à€ˆÑAGNbcu3FGL J0359.7+7649WN B0351.8+7640?ïìÀ.rñ?aáõ®coW?c?Ñ`79?aáõ®coW?îی¶ºÅ?®£Ž2YÚÂ?®¢G6L!ª?®£Ž2YÚÂ?î¤ÚPª"º?˜¼m¢þnÇ?¥²ZòÊd?˜¼m¢þnÇ?ìÑ"ºj­?™0h"Š5Ò?¹vê-øå?™0h"Š5Ò?ï¼L7¢>ë?†	9\–?€ìòŸ'@?†	9\–?á²N50þ?Ё'_F?2?ܛc•žÙ?Ё'_F?2?í=BM#ì'?¡¥Í?¶핖Àü?¡¥Í?áÚ=?·áÙ6X$Ü?ÜK×Õû…Ù?·áÙ6X$ÜAGN4FGL J0358.9+6004?ﴅt.â'@°ºë#À9§)£gxµÀ;®êÏS)@X¥¨¼@}ïAkÛ?ÀG3å?ÄÒU7iù™@(
%ïû@Êú~5åë?ïõâlvK¿Ýˬ&w
¿êãÁ¦(U¿à‡‡émíC¿ïòÄBº³?îI"~Q¿AGNfsrq3FGL J0358.8+6002TXS 0354+599?ïö§Î÷±?TÒ\~ê~?Sà°TR.ú?TÒ\~ê~?ïì9­(uH?nµ1f\?cÆR•'8¨?nµ1f\?ï~ÆË(?‰—˜¾FZ?.7Gc?‰—˜¾FZ?ïü"sÓÈ{?(ВÄïÁ}?;ÜbfQ»Ó?(ВÄïÁ}?ïÓÝ/E'Ü?.nÏ'ÝJ?vhQ‡åó?.nÏ'ÝJ?ïPÞ걏/?¡Ÿ•/rK†?•ä"«…è'?¡Ÿ•/rK†?í
àÛÍp·?¨~טÐt?·ù!&†Ì?¨~טÐt?ïì³Ð³?UoiÓòW?c€L
5n?UoiÓòWAGN4FGL J0359.0-3053¿í;`æÜÀHŒ¦ YŸÀ:ÖêedçÀ<«nñOc@ GʏÜ?ý¶¡è´?Ã,hÿ?³	ÊÀ>Z??ñ…Žd²1@@ó|ç‡8C¿ïþyzϪ?ïöþ~ö€$¿æ";ßT8ç¿Ó0êÄ.™¿á7u‰Ââ¿ØKéBNY)AGNbllNVSS J035856-305446?ïÿ'J5>þC<ۉ?­"'Âz>þC<ۉ?ï÷]4
£­?RRmŒ%·Ò?QE˜³¦"?RRmŒ%·Ò?ï÷ú}薵?Sέڑ¯?PÔå¥?Sέڑ¯?ïý0/¦>v? 'o…5Ü?6~'Öbs? 'o…5Ü?ïÿ‡ÕÕg¯?¦–a_?
€<Ýê?¦–a_?ïÚjf†"?tG'@Y[?rÊödÉùÌ?tG'@Y[?ïö=¼y™?d[(sÕMo?S"†Ö×[?d[(sÕMo?ïöúkҝ-?Dth§RM?R(MÇU?Dth§RMAGN4FGL J0359.4-0236¿á·>"ØüÀCk=ÀTïFÀ;	3Ê1çÚÀ<gjÜì¬@!z²Us¥?úûÏÔ¿	–?Ñb{ö£ð?Éë~:R?üf\Ukl`@¡:ãUÐ?ïvé¡éÜ¿ïÿYM»?ïÿ¦=ìʙ¿ä|{±QFD¿Ãt0é×ʂ¿èèß½jY:AGNbcuNVSS J035923-023501?ïü´vØ?0i'$BÓ??
[UÊjW?0i'$BÓ?ïõSjÛÊ?TÎô L?UYó=,<?TÎô L?ïÐÚòežÑ?t*ªè]¹?w'†¾Â;X?t*ªè]¹?ïè0ªåá?U­xD«õ?gÏTí'G?U­xD«õ?ïø…'FÀÚ?Gunݎc?Mëbg¶ê?Gunݎc?ïÕZ{æ?€¯ÄæpÚ?ur|ÇÃLí?€¯ÄæpÚ?ï­nwÕh?"ó› Yý?"¤zoÉÒ?"ó› Yý?ï½×ßO†P?wÕÒPm7?€Š1õÁô?wÕÒPm7AGN4FGL J0359.4-2616¿ï"«.*ÆÀH>›A:À:¯8lÄNÀ<k5îÏV@"÷Ô7z@@J@Ejm\?ńüéõýs?¡ˆ6ð¬ûÌ?Ù¦:ý,)@++àÖð?ë:kkˆå¿ãó$Oj¡_¿å··6¿àŽ4á‰t¿Üõ¡'FA¿ïïуjƒAGNbll3FGL J0359.3-2612PKS 0357-264?ïü4æ³ö	?6ßú^Á?>XÉ	C‰k?6ßú^Á?ïõÅs´z?TYÿíŒé?Tu
~»G?TYÿíŒé?ïìög>ÂL?còMçËÊÿ?c	˜¬ Ã?còMçËÊÿ?ïönjۄå?7"£.þy"?S#*¶é´Û?7"£.þy"?ïøÜž:¹?BxXˆÚ"?LŒé	HN?BxXˆÚ"?ïÚóÿQë?s.¡7LQ?r÷†t&?s.¡7LQ?ïâûÏ]—?tš¡ÅwÄä?m0}T¡8?tš¡ÅwÄä?ïÐí'âg¶?eY{ÔZ2m?w‰6q??eY{ÔZ2mAGN4FGL J0359.6+5057?í†2±O.¿ùqé¼ÇœÀ8$
!¼À;.•>Á@hDn
B@ÊâçÁE?§Hÿh^?¿×­?W@E™›@"Ÿe‹u¿Û­øᨦþ¿ãwµxó0å¿çlÜ×ÜËH¿éw>û¾R¿ìƓͧ¾¿ïÿ¸SåZAGNfsrqNRAO 150?ïøÃ{ã´?GµB׋"ô?LòÒš?GµB׋"ô?ïå¥<ý?vj%ž"??jZþª‹¬?vj%ž"??諾áÕü?—Ž'Ð7ës?Ÿê¨J¤xw?—Ž'Ð7ës?ïþQŸãhM?¤e¬2Or?*åýшJ-?¤e¬2Or?ïó%¥g>d?aŒyøñH?Y´´°Qé?aŒyøñH?ïë˜qp?©ˆ·%	Ô?œBŒüÚ?©ˆ·%	Ô?îû½¹ðW?šj\šS¶ˆ? D$]‡Ž?šj\šS¶ˆ?ïø½`ɍ?B—£ž^¼?M
|¸Ý?B—£ž^¼AGN4FGL J0400.7+3920?ڗ̌­o\À$o"5ÒIäÀ:-idÒÀ;£J@·?ñ\¤@н¨"?ÉӎG€ó?ÓãùŒ|{?öWþ>^à`@&èãÙ®³?]ʶr¿Ó;Z^›@ä¿Õ9ÐfqN¿æ`MÈá¿êÔ­kÞul¿æ¹£Ÿ×Ì/AGNbcuGB6 J0400+3921?ïÕà¥Oc?š"ä³OK?ŸeCð}}›?š"ä³OK?ïÀ3ŸÖ÷?Š'mµB?æ0kÄV?Š'mµB?í\}²éû? ßÏw5¼?µm0~$? ßÏw5¼?íåö¸iώ?"›¬?°ÐJ=w?"›¬?髑^Îë?¾`"O/"?ÉQº‡ÐÄS?¾`"O/"?îÿ«ñ­NO?¨ïs›w? @蚷?¨ïs›w?çlÙ0¢#?±èÑe7è$?Ñ&Mž»¹Ì?±èÑe7è$?çñ˜x?±¡CZhn?ÑøÏÍñ?±¡CZhnAGN4FGL J0401.0-5353?ïÂdÊÁÀG*UC(s½À;NXø¿™ÞÀ<Ïq¾‰=@!í\MÞ°$?ùr_µj?ʏ˥†Í?°Io	Î
?晐?'Þ@ƒtük¡?ï×£ -²k¿äRW…øÒå¿âW˜" ;_¿ÖÐ5'BåÙ¿»F@V1dý¿Ó5½|!åAGNbcu3FGL J0401.0-53591RXS J040111.9-535456?ïþç‡kÍ6?Éêþš]?!‡…%וÍ?Éêþš]?ï÷CÛnrœ?S~¶àý?QxHØã8Ð?S~¶àý?ïõjïH]ù?Tlqs,îÜ?U*!Ý7'?Tlqs,îÜ?ïýšC:?­ƒ~ÿ¢?3/nuÌtÎ?­ƒ~ÿ¢?ïÿ/ú³SÄ?1«Ý´á?¬Ê??1«Ý´á?ï݄ºOi?rá
Ý÷_"?q=ø¼EgR?rá
Ý÷_"?ïöì@¹W?aµïø¸Cl?R'~©ý?aµïø¸Cl?ï÷=?ÀN(?FÂôgÀhK?Q…€q¥?Ý?FÂôgÀhKAGN4FGL J0401.3+0412¿è­'¥¸XÀA?Ú@RÖgÀ:>¥¸‹Í(À<
ïGK@7A"@±¤RZ@?Ãq·<íœ%?§cm1µQ?åujæ'è@y&
«ª"?ïÿµÂÅ¿éæ)«0ñ¿æq´]j>b¿àïÔ;V¿è°a&‹…¿ï÷¡Œ­"
AGNbcuMG1 J040119+0412?ïù%üqˆ·?D¨8ÊÃF­?Khfdà ?D¨8ÊÃF­?ïô,2õ
?T±þY·?W§š‰fÅ)?T±þY·?ïÔîC%U?w=¨Ä½.S?uðÄPMµ?w=¨Ä½.S?ïê4œi،?I¹:ôäo?eËcØóÝ?I¹:ôäo?ïòTMV—^?]jç£<ƒˆ?[WeÆ?]jç£<ƒˆ?ïÖ@fTž?thÞ '¼Æ?tß÷¼W'9?thÞ '¼Æ?ïfYd0'U?¸m¦=ð:?"4ÓyíµX?¸m¦=ð:?ڲŠú?w`'6‡õ,?Ž	]¬Ž?w`'6‡õ,AGN4FGL J0401.7+2112¿Íñ-ÙpãÝÀ7?uÙ ð¦À9"a#0†±À<ä)à¤@ŽzÒ.5@G6¥®zÒ?±a¹ƒnßÝ?™";$³Ž?äêׯ~Þ,@9¤=Œ}|?¢0ž@¥ë¿ås´È¿çb P‡Ø¿ä¥U~Ž¿å°ÉaÕ¿á=u¬T‡AAGNfsrq3FGL J0401.4+2109TXS 0358+210?ïÿLgGô?®Ýè?ös°ð?®Ýè?ïö¿Ä†9?T–HÊ:Ú?R€wÜrî?T–HÊ:Ú?ïöVápÚ?@"ÚCJS?SSçõ¦l‡?@"ÚCJS?ïÿ§âi>÷
ñ]ä£Ð??…{ž>÷
ñ]ä£Ð?ïÿW4UƒP?
6NË'Cÿ?p¿ç†?
6NË'Cÿ?ïà…‹ðŽž?s …Êòd†?ozt8¬±ß?s …Êòd†?ïòדOR¤?aå⣝ÜN?ZPÙÇ(Q?aå⣝ÜN?ïÿUӜÚ?¦îöáÇ?E'?¸Éõ?¦îöáÇAGN4FGL J0401.9-2034?Ç{Yι+ÀG3'äKoÀ9Žn™:Ï	À<]ʹÍÈ@UBø";@'<O;§v?¯Ïbpãm?¬© Øà?úð¥)œ±@1ûЛc?ïîíôdÁK¿â*^x[[¿ãµo¸õs¿ãa.A?e¿ê\w?&±p¿æ=¨6ëN˜AGNbcuPMN J0401-2034?ïþ`ñ1†
?¢j"Å È?)ðê½±´?¢j"Å È?ï÷ö×À?Sº}Žþåi?Px'ƒ:àŽ?Sº}Žþåi?ïåû;KÓ?q4õX³<?já²Ö5:?q4õX³<?ïÿ)0ÙoP?,ëw[ û?Ùì¾k?,ëw[ û?ïý1dãÉ?0Òó•e ?6t×ä÷¶?0Òó•e ?ïÜýÆaE?~ËêП?qø6<yA?~ËêП?ïÖ#[µïw?{'eO¿uÁ?tîR{ ¾?{'eO¿uÁ?ïþ×G5Yå?6"6ÿ?"‹mÁ?6"6ÿAGN4FGL J0402.0-2616¿ïþ¯9'Ç_ÀG׍÷¤ç«À:'C‹p+À<4–åŠ2ô@•§vQ?ÿëî€{»b?»§•/Ҁ–?ÅÒ.
ªRú@
«Ý3L]§@†Êk°??âk6¯Æ,?'‰ÇПÑR¿ßˋ¤cw¿á‡Öޞ†h¿ãxUFƒr¿ïûþ~ÀAGNbll3FGL J0402.1-2618PKS 0359-264?ïö…5'Â?[Xåt»u?Rõ•Wk»?[Xåt»u?ïôvPƒ?Sȹ"&
?W^ãÚjM?Sȹ"&
?ïÛõö"ç?n'zwÏC?rß&Xg?n'zwÏC?ïî?£S?D6/D÷0?açÀ}çìù?D6/D÷0?ïòAdèü?YdZ¯cY?[}5ù̶-?YdZ¯cY?ïÕg	ÆÊ¢?wL ÀA¡?uL{3ø?wL ÀA¡?ï:í*ª?»FÀîB?¢Zª½Ñ?»FÀîB?ï²aIæ9?mCÛ"å?ƒgœ·}O¢?mCÛ"åAGN4FGL J0402.0+2737¿ï¦nýlZzÀ2¦•BCÀ;yD|	À<[Òç™í@¶†ƒ<`@`Ù¼ŸX?Ê(y›ÍP€?¡Ìud8#?ÚÛÏÊ@ÃŒÜÇÂ?îÏËOKE¿äùˆaãÊÀ¿é.f f¿å+§'i?‰ÄÔcw§4¿è…#ÀÏhˆAGNbcu87GB 035856.9+272842?ïþLjM	?#Ðþ/\5?+9^_æE?#Ðþ/\5?ï÷ üW‡"?S|þ°Vì?Q¾i®'ò?S|þ°Vì?ïñà"r¤@?e1®H\K?\?»ˆªÿ‹?e1®H\K?ïþŒR^F²?XbÖi€º?':Úî°
þ?XbÖi€º?ïüØ-܏Á?;5íHßFô?9>'0•©€?;5íHßFô?ï؝l{Ã	?wëÚA(?s±I®0¿º?wëÚA(?ïå¦'úùd?ue£3Pƒ^?jYØBߔ?ue£3Pƒ^?ïôUךRž?PÙkr"+?WTQG²U?PÙkr"+AGN4FGL J0402.1-3147?Õ&4¥ÀHEmã2iàÀ:OŠÞó­À<œ£Žåáq@nf½¤:Ý@D–eÖô?¸q¢"¤¿è¿‹è	û<²õ?Òm˜ŸH°@úþ½_Çf¿Êop»©äÀ¿åƒd£î‡¿æ=E¥ü~k¿àŽ1@¿¸½¿æä"pB]¿ïÿÿ" 5•AGNfsrq3FGL J0401.8-3144PKS 0400-319?ïþQ$ñã?Í@‹­!º?*í¯?þ´?Í@‹­!º?ï÷…+	?PÆk¨«?PõÊkw^
?PÆk¨«?ïõU+¢èo?V¬QbäGÞ?UU¨\¹Â?V¬QbäGÞ?ïünȊ?&Ó"vɀ?<8§µ®??&Ó"vɀ?ïýۍ"ãT?%äZj?1#'
Lԛ?%äZj?ïߺ"d—ô?qEæ€éV?p"½Úù?qEæ€éV?ïòyã#ƒñ?fnMƒ?[9XÃ
ý?fnMƒ?ïóҊr#?HE™h^,P?XZë…âê?HE™h^,PAGN4FGL J0402.9+6433¿í±¦k$^@!Ü¢˜E܃À;0uєÀ<Md;é»@!ë×ðÂJh?þZj)i…Ö?ݍ}K…:?¬1ž!'u?¯7Ö°ü6È@œ^;Ÿ"Y?ïûŽ¶çˆ:¿än­Aí
Z¿í~³íQ¿°@ô'âÁ¿Ï^z·¬)¿à¼-BXj$AGNbcuNVSS J040254+643509?ïþ8—=?#ô¦eϛ?,ÛțÔà?#ô¦eϛ?ïï¶[Ç&?_ÎQýcƌ?`I¤Wv?_ÎQýcƌ?ïãIüR?r÷"_0—?l¶êEÚ-÷?r÷"_0—?ïû+ù‹?0*#¨"H?CS²®ÂI?0*#¨"H?ïý<4þSF?5ÿIÚf(Ù?6W©W"²?5ÿIÚf(Ù?ïŸOMg‰I?'ÑT´Ñ¡?ˆ,,¦­Ý?'ÑT´Ñ¡?ïᐉƒ)ž?z~¢)+Ž¡?nov^™Ñí?z~¢)+Ž¡?ïädGõ"s?cÒBç‹?k›·ÏbDî?cÒBç‹AGN4FGL J0403.3+2601¿"¨^ýœÀ3—®FÏÈ*À:uêe:íÀ<"Š•Ø@—ÿ-ól@D@¡±?Éò–J"³ƒ?ÑÕÍ\>Å8@ÐP_"äN@½¤ܘG?ïþÙY£	…¿ç®yZ^ñ'¿èǰބ°(¿äßS¢"j¿ïÿ÷!	:?áê8ÅCAGNfsrqOF 200?ïØcq"†?'O•||?sÎGbømD?'O•||?ïÌ_¹ó·?'Ái´}	f?yÐ#nÇp?'Ái´}	f?ïc*(6nÁ?†ªÐÜM‰¦?"šºòRïñ?†ªÐÜM‰¦?f±ºÎ?p‡é¦žÑ?Œ^¦d¿X?p‡é¦žÑ?ï¼jÊhˆ?ƒ6:–(FØ?€å~ãýØ?ƒ6:–(FØ?íù¸hð7?²ÏŽÀÕ?°7º>pLE?²ÏŽÀÕ?쒭¯Ùª‰?¦…*óYå‹?»j'2«µ?¦…*óYå‹?êÉHrŬ?ª¤3é÷?ÄÚßÆ4éR?ª¤3é÷AGN4FGL J0403.5-2437?ãè ÍëZ×ÀG{SÞ¤e¥À:|%«‹3¥À<†:8
3@Fëˆúÿ@^®&˜}?¾x2–«'¶?"Úâ»x3?Ò)["æ^ï@

åÓYü¿ÛÖPē˜N¿ãòT{'W^¿ãn=Mh¿ét÷Ãñ[ø¿ï¼jÿR[?îÔ1°|4.AGNbll3FGL J0403.7-2442TXS 0401-248?ïþ–ã? Žü}ÑÍ?&Ÿþ[dӈ? Žü}ÑÍ?ï÷ŠÆp<?SAš½¥¤T?PëЖÛw(?SAš½¥¤T?ïÑ ÊX†Ý?yò¶€WÍ?wošÅN5f?yò¶€WÍ?ïþŽN?†±?½ ¿v~³?'4yº?½ ¿v~³?ïýa$æœà?2ë¨Òä5?4öØ'E98?2ë¨Òä5?ïކvY×?t)U?p¼Ä×3ý¹?t)U?ïÖÝV5?~Š&íÿJ?t'TÙҕù?~Š&íÿJ?ïù¿Ðv5Í?B¢zÃA!´?I½&laÕ?B¢zÃA!´AGN4FGL J0403.9-3605?àí¨_/:€ÀH=ÄڐïÀ7R}hájêÀ;¤eƒèWm@j/™@%Ø{V¸?'»˜¼'…?Áœa_–h@*9AÈ!la@!lð—'=2¿Í`ž—i¿âäZB@Â=¿èt¤Ò²À¿éj šª:Ò¿í@j‰
Ö¿èãD]}¿AGNFSRQ3FGL J0403.9-3604PKS 0402-362?ïàÒ¿ÄÀS?…hÆwzO?o-@bõx?…hÆwzO?ïϨî1‡ž?ŒŠ<!¾?x+ˆÜ=q:?ŒŠ<!¾?ì償j°?©R¬ÅýB?¸ÓÛý?©R¬ÅýB?ïöM³oa?Zráv)3?Sdà3lÎ?Zráv)3?ïЬƥžé?tµx´3?w©œÈ­kN?tµx´3?ï-ð$"ˆ?²z,×N…õ?šAûm·"?²z,×N…õ?îZ|}©ùä?¡ÁM¥•ÊY?ªX8)«äº?¡ÁM¥•ÊY?ï9ÎzC_?‹ /Äé©?Æ2ob?‹ /Äé©AGN4FGL J0404.1-1715¿î@¶²ÚÀFJ5çB™ÙÀ;CTxþŸÀ<Ì۔ìÝ@ )–ˈÿî?þïÙ\'HC?ËÅPV¯$?«—á€"‡?âTŸ^Õxm?ýQµ§—38?ïË$V ž¿ê‰G;þ³Ð¿Ï¨£¸+€¿áãÚÀ€c=¿ØÄúptb¿ä_@zAGNbcuPMN J0404-1718?ïý:4Hî?eCeÎB›?6.]'¯×?eCeÎB›?ïõ"cØ­?V¿ls½R?U»8ÃE…Š?V¿ls½R?ïìÓ,És?q(=¶ÄÍ¥?cì-$Ð?q(=¶ÄÍ¥?ïó —ÿTx?;כšõöÚ?X¾ÐW~?;כšõöÚ?ïþÔᐠ™?/ë=ÏÁ?"±ã6²?/ë=ÏÁ?ïÕ«/e•¨?x|gK•?u*hb'¿­?x|gK•?ïî9E¾G›?r$à"ï?aƺS–\¦?r$à"ï?ïÏè؊à?ffëL¹Ê?xrÜ˜+?ffëL¹ÊAGN4FGL J0404.3-1559¿Ñÿ·ð
®IÀF
–_RuïÀ;O²——aÀ<ÁR¡ƒâ@Žèc¬!Ü@qL"îA'?Ô{Á!Gù>?Ó,Kb~û3?üBkK @$ñ[Í[=?ïëÁ¹É:?Ù-«ŸU›=¿åSç]DZZ¿×õ¡Ø,|¿ïÿúŒ—Ó¿è—Ý÷vÅAGNbcuPMN J0404-1559?ïôRcéÎ)?R1WÂE‰?W[8(]Õ?R1WÂE‰?ïòÇWdbM?Y›ß¤œ?ZqP¾I'l?Y›ß¤œ?ïyNÿ}µI?"X†§Å?Ö $ç?"X†§Å?ïÚ\
X>l?Uz)_ŸuÅ?rÑùrÍEü?Uz)_ŸuÅ?ïö»…ý…|?P
"½Ð?Rˆó†ƒh?P
"½Ð?ïÒ¬»'ñ<?w¿Öy†Å%?v©¢,8Ó?w¿Öy†Å%?ïDSÔ¾]É?'Õ/ðµv?—u…cÜá?'Õ/ðµv?ïoÏ^€¢?~î4³B?'6Ûý?~î4³BAGN4FGL J0405.6-1308?ŠšîÆÀEPíÍ9ÚÀ9wdå\æ‹À<KãýjúJ@oâ˜»ù@sÞÚŠ¬?ª»=RÏ¿ŠYE¢Ë?ÛÌӂÉs|@ƒæ2(œ¿Ùʦ¢¿¿äœ´&†'¿éz¡†Íå¿ä9Qàd)¿ïü'¶vI2?ï×i©âAGNfsrq3FGL J0405.5-1307PKS 0403-13?ïý©÷¾E©?(¾Âè¹?2°CT`É?(¾Âè¹?ïøNè	X?Onº'þ8´?NÄ_CýЗ?Onº'þ8´?ïÔÂÄ­ê?{'3ÚOÒ³?už¶F?{'3ÚOÒ³?ïÿÔb²?œ8Õ¥ÒÉ?
ñEò¡?œ8Õ¥ÒÉ?ïþW2ä%P?+E›ô*ä?*ŒÒW™x›?+E›ô*ä?ïÜáU×K?s¬ÄOjîV?qU#š"N?s¬ÄOjîV?ïÚ©ñÍڋ?|Ô9':â>?r«2Ö8?|Ô9':â>?ïþ³nVö?(N*¼^n	?#ÔÅ D9?(N*¼^n	AGN4FGL J0406.0-5407?ïÒÞO3ÍkÀFȒ£"¯À:àŸd´µÀ<±2«M÷@«ó[VèÅ@¯àè@?Å
ÈÂ|?¤Õq¶ü€ï?à_o1CD@?ûH
ZÍ?ïæW¸M¹Ç¿êË
å›Ð«¿ÚƒÊE‰ø¿ãð'~Êá:¿éž%"ôÆç¿ïÿý±q&´AGNbcuSUMSS J040608-540445?ïøՙ¥.?F§ßÕ?L©˜¦š‡Ø?F§ßÕ?ïöá"&Š?TË?p»¤e?SÀ=Måzf?TË?p»¤e?ïÈ4+x E?|.Lí
.S?{åê;°ÍÃ?|.Lí
.S?ïô"¤ór‡?@wa §œ?Vöµ (³Œ?@wa §œ?ïè¦tÉUŸ?c[¹èƒ1"?gY‹x¢à¶?c[¹èƒ1"?ïÝ°_r›?qçI"5d?qt§¿È'‹?qçI"5d?ﯦšÍºø?†¿¯ØË?"YGÁÍý?†¿¯ØË?ï×BT–ãº?büã6XG?t^ÕÔÚv§?büã6XGAGN4FGL J0407.0-3826¿êáÖî(ÀGð:}ªOÊÀ8'pûëžIÀ;ÌÊ÷à@ÊÊÁ¯¸?@øfC*÷û?£w£%o·?¼¨ËæÙD@ÿE™›@Y؍Ë/>?èP«Hî†[¿ÝJŒL˜_¿åÏÞú÷­¿æ^ä&…¥Ç¿é!(n´¿ïþ'jöîßAGNfsrq3FGL J0407.1-3825PKS 0405-385?ïø:€?Gž"ü??O}p3¬?Gž"ü??ïôðÁ¸`s?X¡î[Η?V|¸ziÚ?X¡î[Η?ïĎGßpF?q¸joSƒ?}¸ÜXá?q¸joSƒ?ïû¦tH|F?0»m	–?Af.Ö\–T?0»m	–?ïö‡OÛ,?P%‹æôb?RñÛeÉó?P%‹æôb?ïÖq;àœ?!`3,¹X?tÇb1§ÝŸ?!`3,¹X?ï¹m&ŠÎ?ƒw1rí+?¤¶|Uw?ƒw1rí+?ïðŠ2.·Š?Pu†ä1?^ë›ÔLf?Pu†ä1AGN4FGL J0407.5+0741¿»÷¥œòÀ?$GäÀ9U¸éÀùZÀ;ëŽÑ¿zÕ@Ç=ûc84@Wn{ޝ°?°Øú''–ñ?£(:[ÆzM?òqV8ú@½Œqg÷5?î 'ódK¿Òý¼-î%¿æºUÑ쓿ä5ëß·‹¿âû"ÀĀο倴%6nAGNbll3FGL J0407.5+0740TXS 0404+075?ïþi˜R¥G?c›°§@?)fw$)?c›°§@?ï÷«û›í1?PÃß^	U?P¨	ž½Ë?PÃß^	U?ï𛄼xþ?`
ÎJ³O÷?^Èö$Dâ?`
ÎJ³O÷?ïöc€qÄ,??‹§#c"?S8ÿ|¬¶È??‹§#c"?ïüø€§&Â?+ù֘֟G?8;úYïçi?+ù֘֟G?ïÛFTÎ
•?~¡ûIVE?r\՘II·?~¡ûIVE?ïèy‡f¢]?qöUÏÅƍ?g†x³z«??qöUÏÅƍ?ïäIýúí?[#JXÐèò?kæµýåŠê?[#JXÐèòAGN4FGL J0409.4+3201?Ñ­¬¥SÐÑÀ,»"F™A…À:j«¾_KÀÀ<L)'ÉÁ€@ aùkç.Î@XKä ÷?»`¥_?¬¿n!¤H&é?Ö`½Z?ôÁ­]è?ìw~¼ž¿ééKRä©b¿àA|lb(ê¿Ó†_!£"¿à`¯"#¿æ'z-ǪAGNbcu3FGL J0409.4+3158NVSS J040928+320245?ïùa¨Â?A+¹RÚ;?Jy_è|Ä<?A+¹RÚ;?ïéªFB¸?g°ê>ZØ6?fU¹ð"#®?g°ê>ZØ6?ïëPó"é×?h
ÄDƒ3Ç?d¯n·'|?h
ÄDƒ3Ç?Käãx?kŠ ™qb?ˆšlõ™3?kŠ ™qb?ïôéAÞ­Ü?M½ë…‡?V-|—Ú—†?M½ë…‡?ï³UNTæ{?‰)V]?ƒ*¬z"•'?‰)V]?ïë¹Ìadk?p‹?¤³»?dF3m!4é?p‹?¤³»?îÿþ}sô?'x5'tk"?®p¼u»?'x5'tk"AGN4FGL J0409.8-0359?܌"Ž'ÞÀB°€Ç:¼"À:0î'hÀ<K.cÀ™¹@¯'aÁæë?úօ˜ZÕ9?ºê!Fv²?ÓÛgšC
@ý+¿¡k@ö0툯?ï—ÆZÂÄ5¿Öµžþ'U¿Ë"Îš¿ßW
:M"¿ç6Ë£×àý¿ì+½óëõ‡AGNbll3FGL J0409.8-0358NVSS J040946-040003?ïԁÚ`3F?uEeþu0?u¿ÄçœÐ?uEeþu0?ïóª¥Á¬C?WENÉA?Xªµ˜xR?WENÉA?í"Ðýç‰?£êÓÚô\þ?³ax1÷6?£êÓÚô\þ?ïâ8— B–?PWSG³L@?mÇhÄêµ?PWSG³L@?ï²Õ°SÎ?ƒÌx²LýŒ?ƒ~ʚX~?ƒÌx²LýŒ?ïÓ̽ª½P?wïEˆ£d¸?v¡0 ¸?wïEˆ£d¸?ê½z«n?±¾V]zr?Å
QÂH?±¾V]zr?ﰃ³~G.?nWkK{r?ƒß>èš?nWkK{rAGN4FGL J0410.9+4216?ê·f»ÎÀ&Üã›EÀ9t»=¤¦À;é?l&š@vI±ú¹o@ËN˜‡œ?¶®#ÿ¹‰#?½ÞúaZë@î"þ"?@X1` (Õ?ïµK;gµ¿Ÿ¤,€Í¬¿â<à<Z¿âÊ|ûÔ!U¿â¥É㽿맾ŠßÂAGNbcuB3 0407+421?ïþ›ª"½?$]fגä?/ÖCöpS?$]fגä?ïðõi+Æ5?`0՗—ýà?^.hU_?`0՗—ýà?ïî©HÈß?`՛Ƥ#?aV¸9±?`՛Ƥ#?ïê­*p?Jø†È×y?eRÕË5?Jø†È×y?ïý*ÍÖZ?3î±êc?7¦ªãó~ ?3î±êc?ïšìÄ ?–ÀSê'C?‰~Õ·3?–ÀSê'C?ïÃAozÐð?×w4d•?~_H?'ëÔ?×w4d•?ï¾íûEÂ?i>=‹"sÍ?€D»¦
j?i>=‹"sÍAGN4FGL J0411.7+3041¿ëöÇ{Ã߂À-ó—»s5À:ÃÑðøüÀ<#AՍe¯@mqÕ‹@pÈ¥ߙ?օÞzt:?慍Þzt@oçáüú?þä#›e¡š?ïäÊ"%¼?´'ÿ¡‹U‰¿áˆÞ@<±¿éÆh¸P>¿ïÿ}#AM¨?ïû?!ÎAGNbcuGB6 J0411+3040?ÎkL?°«¶"X÷?¥Õ®dÎ6?°«¶"X÷?ìWdf˜ ¯?¾ö´ý£.n?½DÜË>ú‰?¾ö´ý£.n?ì9Â6ï?¥"«%ڛ?¾1îO(‡3?¥"«%ڛ?è'x2hÔ?¬_¬éї?Ïb7†\¯?¬_¬éї?çØ]<
?Ìsh—îô•?ÐOýE‡ëê?Ìsh—îô•?׶!ä½k?҉U0U±?ä$¿o
¡K?҉U0U±?æ'3¤$ë?¸NÈïÛ`?Òûõ˜·¶)?¸NÈïÛ`?ÂH¨~"?«nÊÚv‡?ë|-Õü w?«nÊÚv‡MIXED4FGL J0412.3+0239?àŸv…mg·À@™3]$žEÀ:4±‰zg¥À<³˜H`Â@r_˜ìË@b%#¥÷v?ÁZÌ)cь?®@Ÿb4?î"ЧLàƒ@3U#‡¿ã¿9+
Ë?Òµ)­xs¯¿äâ~—_®¿ã Þ҈Îp¿êŠDý`¿Þy–ÄÓHAGNbcuPKS 0409+025?Dka?·S`áÀo‰?ˆÕX®å'¯?·S`áÀo‰?ïö*¸ªÞ?S(·þOæ?SªŽ¿
m?S(·þOæ?ïđ&˜??¼Ó_¿?}·}9üwù??¼Ó_¿?ïñ™Â«®?A l5e‡q?\ÌzÁa±?A l5e‡q?ïå'!,™?l-	>hS¥?jØÞÝOQ?l-	>hS¥?ïØQéè͛?u}Ýs1©²?s×
ùNÓ?u}Ýs1©²?¶ïs?Œwp0?^;U³¿?Œwp0?ï·»|(«¬?pÁå(>0?' ò½o?pÁå(>0AGN4FGL J0413.1-5332?ݔЃÝçõÀF\Ïkã}éÀ:‹…ÛÀ<QäJ—ÓÇ@±Šû"@/«SÖ@ê?µ¨Á?O÷?—°þ‡|X
?á`fQÒ@Ußêáµ½?ïÒéçÆ²¿âIfÿQ"¿çVSÉ«°¿åH¦4¿è|z¤áÌ¿Ý·Oµò–AGNfsrq3FGL J0413.6-5334PMN J0413-5332?ïÿ+…?	5eýƒƒâ?Ÿ>tð…?	5eýƒƒâ?ï÷̦ûñ—?TD"um¶V?Pf±"©ò
?TD"um¶V?ïõ"¤Õ´?T§PÕp5x?TÖ··ZØe?T§PÕp5x?ïÿÛï÷Á>┫"âz>ò©—qI>┫"âz?ïÿ^ÉTj?éÚ¬"?&ãžßŽ?éÚ¬"?ïá\Bdî0?oDŽ§±‹?n£½µ.×Î?oDŽ§±‹?ïí'ðF¾D?f·å¹rœé?bnÔ¾›¢?f·å¹rœé?ïÿÉåÍàÚ>ñpõP¢×>û
0
fž">ñpõP¢×AGN4FGL J0414.6-0842?æς^¿~ÀCW¼]éÀ#À;W‹àsr¾À<§ü­e(y@àoW%Ö©@æ—b%?Ç鮄ã)0¿…/n=Üj¶?¿a@Œ¸	Ç@›2֖û?î©z¸-˜¿í;ž§"?'n6'ž¿æ¼ˆabñg¿âÙA…Þ¿ÔíUBý€ŸAGNbcu3FGL J0414.9-0840NVSS J041433-084206?ïþp¬C?!'ÙèóD,?(õ9qs‡M?!'ÙèóD,?ï÷5¹lÀ?Sá_˜¤K®?Qהê›ßV?Sá_˜¤K®?ïôצ֪,?YÛ>XÃú
?VP²±çb?YÛ>XÃú
?ïýRËvX?ªÙüYb?7i¤M@"?ªÙüYb?ïþMfê‹?$í@m×í?+)Ï8]®?$í@m×í?ïعì³Y?€VI,€¦Ø?s£	ùËN?€VI,€¦Ø?ïö¢à%€S?fžÞ
{Â?Rº@ 3(°?fžÞ
{Â?ï÷Yx|>?BšFp Â?QMÊûÉ´ô?BšFp ÂAGN4FGL J0414.8-5338?ßñ»"o/}ÀF9Ç͉‹/À:ß´tç2ªÀ<ŒZ{v™@!Æ.Ü"?ú¿$º|?Él;½pc?Âu	ÂK"~?÷Dî|Iýz@¾ØR'ó2?îQí}ÇV?×/!°ÿ½¿ÃW—ULj¿Õ]ä·¥¿Â®9#b/Ë¿èg²GcAGNbcuRBS 0526?ïýê_•øá?#þ«˜´†?0­÷){Ã?#þ«˜´†?ïõEü'r$?TÎ3!b?Ut®\¾?TÎ3!b?ïïžÜ#¬Ø?aäU`IãÄ?`a#öp/v?aäU`IãÄ?ïíîèÌ÷?Jÿ»ç	w»?bÿEí¸f?Jÿ»ç	w»?ïøgl˜&?F~=,7>Ñ?NbNp܁í?F~=,7>Ñ?ïØ®Ÿ\ž‰?vÖǤ±0?s¨°9£w¯?vÖǤ±0?ïëYwÀ€ä?n+èõ Õ?d¦ˆFLB?n+èõ Õ?ïÇmåE!?p‹1QÔ¯?|I
~Ýov?p‹1QÔ¯AGN4FGL J0415.2-5741¿ÙošÑ–ÏÕÀEŸaܓê-À<1 'EÀÀ=Gýœ@#`ãÍDkë?¤=Æ_u;?ä':l˜•?ïüšò?ÿÛÄ?þ©úE+¿ïþæ?d™Þ?î¹NjÇ7¿Ë©nù²Þå¿ç8Ð@Ô?¤0Q<Ľ›?Å¿ˆÁ…AGNbcu1RXS J041505.7-574237?ï"P¼Ûèô?¸ÄÃÕ1"?ŠëÐÏäúÙ?¸ÄÃÕ1"?ïö¿+#š?S¿ýgéƒ?Sæ6Eì.?S¿ýgéƒ?îz9ë;ÖN?›&{€.,œ?¨\aJŠÍ*?›&{€.,œ?ïù6#lZ‹?Ep²`Lð?K'qíÔ»?Ep²`Lð?ïÉÍz¶nU?|dÛÒô6"?{B³71;?|dÛÒô6"?ïÏt5B=M?"ËèDy6
?xEå{¾?"ËèDy6
?î d0x,?›QúùÊ¡?¥ù¼õaE?›QúùÊ¡?ïø7_ÎØÒ?Vo^Ã°?O"€¢†ÿZ?Vo^Ã°AGN4FGL J0416.0-4743¿ï´|è3IÀF½#N¹¡wÀ;fÞõÄ<ÛÀ<ßùË2˜Ú@Nšþsì@xä$Ø&?Ò-úNw\?Ë!É(}w¥?ø[Ƶ[—@(¦h´õ@?ïù–Ys8ݿތ¨ðN²¿ç›Ê`áÂ'¿á±§­Y¿ïÿ¯Èe_¿ëý€Ú†AGNbcuPMN J0415-4737?ïù«îc~??ò¬X!ó?IPG^mŽ??ò¬X!ó?ïõþV\®?Uœ×UT¯?UîP†ô?Uœ×UT¯?︭Bî½
?{8˜Xï?Ô¯O§rÌ?{8˜Xï?ïô¯oÍ?<šè¡åÛS?WóöÂ¥<?<šè¡åÛS?ïûcÒ@!?=ý#ÜüÁ?Bs‹ØXΦ?=ý#ÜüÁ?ï×±­6¯j?Av¢àž?t')u??Av¢àž?ïMõ«8Ü?‡Oÿ—†a?–A_"/êv?‡Oÿ—†a?ïƄPS¡à?h"|?|½×ÔÏ7ÿ?h"|AGN4FGL J0416.0-6628¿ëœãˆÚÀCí½Q.ƽÀ;C¤as¸À<»ŸÖÊ|@òs\æ`@Gý'w>%?Â;…èí¿«£~€Ž†?ëIA'¼Á@º•'LC%?ï–T€4éñ¢Íõ¿硑J?¿3¿Ý½"ÅÌþK¿â&¦'¦`Q¿Ô´AGNbcuPMN J0416-6629?ïþѽ³?=%^Ÿ´T?.ä—ŏ?=%^Ÿ´T?ïõ«¼—%?UÉ !ã?T¨ˆ5HU<?UÉ !ã?ïøf¢1©×?<Çþœä?NewôÐ2?<Çþœä?ïüJ÷¨¡'?$Mþ­Ú|Ë?=¨C Zl?$Mþ­Ú|Ë?ïýŸ.¼?-®[?ë?3Œ#ç5©?-®[?ë?ïÙ³©Ôéì?vCцZûŒ?s&+jB4?vCцZûŒ?ïø•Ç–ÆÅ?W3Gêøq?M¨áÜkg•?W3Gêøq?ïæ¿"'!?\SûÜ+"ç?i@ãi®.Ñ?\SûÜ+"çAGN4FGL J0416.2-4353¿âď&ÜÀFðîcŠ	À:ßÇÏ7
XÀ<žÑ0ߛÜ@rØòõÖ[@Ð<eáÜ)?ÆH3
‡¶?¿pQ¡³C?óÖރ®uÊ@a"²VÔοïÿÃ.¾Ym?ïþ­ŸàÛx¿æQìAZ¿ë3^ ò"Ü¿ç"¢^º¡¿ïÿס<%JAGNfsrq3FGL J0415.7-4351SUMSS J041613-435057?ïñ"ãÀëS?Ž­;3žL?]º8‰(9?Ž­;3žL?ïö¤Í‡æF?T?Bü â?R¶dòó#
?T?Bü â?ï¤Üú‰?‡{Q®>.s?†Èû_pùž?‡{Q®>.s?ïýƒð J4? ø"û Ÿ"?3à}Ù6t? ø"û Ÿ"?ïþ–iʅ0?/ˆÄ_.iÞ?&™d–}Ø?/ˆÄ_.iÞ?ïÝD¢­z³?{hJ	@
?q]®» žL?{hJ	@
?ïMþ?"¥_rÍì?–^"Ãn4?"¥_rÍì?ïô˜ÜÜ?L³—˜nÒ?VÏî­®·¬?L³—˜nÒAGN4FGL J0416.5-1852?è'ù2öWÀE3§Å¬À9wc(ÄDhÀ<[²h!@†Ì<Ùû	@ö Ä0F?«ˆ>®ïö?¢ä,å¼1õ?óõãFŒ@Ge€¸L7?Ã_چç¿ãuÒêóÿ¿æ"	\ ¿æ'ä¾®&¿â‡vfœí¿åm¹ Èw~AGNfsrq3FGL J0416.6-1850PKS 0414-189?ïÿ8ýB?	›YgR68?àcÈÏ¡P?	›YgR68?ïøBþ'Q?P×
ÔG}?MÂôæCŸ5?P×
ÔG}?ïöY–|â?Tb
÷«ÎË?SÑLŽNý?Tb
÷«ÎË?ïÿÆÈ—î>ð¢Ðdwÿ>ü›ý
Ü×>ð¢Ðdwÿ?ïÿŒš$%q?¢Sâk'?ÙgÿØz?¢Sâk'?ïÞ%n?rê"0Ìž?pöm<"ä	?rê"0Ìž?ïô=¥/­u?d ¹•*Ó¢?W"µH¯â?d ¹•*Ó¢?ïÿ¦"AKW>þH
1MV?^ûzŸ_1>þH
1MVAGN4FGL J0416.9+0105¿ït—Ò<èÀ@"¢ƒM&úÀ9¦¾r–öQÀ<	¹07Ö0@ rÞÎ,j?þ4rHø"?±en™»¨b¿†:A"ÖJ?×]_A. @		l¥Å¡à¿ÛüÑö®H¿ä¸u\£o¿âkIYæ%c¿Õ՞Bà¿áÔM"ÞHö¿Ë¢‰pîUAGNbll3FGL J0416.8+01041ES 0414+009?ïÿo¥³?
\Ǘ
==?œ'E`%?
\Ǘ
==?ï÷B)U—?Q¼.ØÐÒ?Q{®IÆqæ?Q¼.ØÐÒ?ïøñß¼ú®?[P#b"w?L8â|ç#?[P#b"w?ïýN'€¢?#-åôÌZ?5Ç­y?#-åôÌZ?ïþ€_G?‡õ­‡Ë?'þPJ	ú{?‡õ­‡Ë?ïÙz'?ûz‡?sBñ"iøl?ûz‡?ïúî0ß?GÅx}¾¿g?DEü+顝?GÅx}¾¿g?ïùÜ~µV}?9ÇÓJH:?HŽ"3£·?9ÇÓJH:AGN4FGL J0418.1-0252?Ò¥†Þg:2ÀA…
¢q›À9Áíûñ}†À;ùôñ¯e@FÔ¸~Œ"@(N?þó'?¹5T`)‹j?ÈOFúTv@
d8Š‹	@™—‹wlô?ïÿ >ybm¿á¥ø¸
"'¿ãm9ßtÅ$¿ãéíÚcŽE¿ìo>±ìv¶¿ïþ–]úÝAGNbcu3FGL J0418.0-0251PKS B0415-029?ïĨ-'¢Ô?{µ#§"Ç?}«éy=?{µ#§"Ç?ï÷
cH'X?S'[l¾Á[?Qå9 u®ë?S'[l¾Á[?îøU¼ ?˜Z»Ò~;?¨z¥íÍ¿?˜Z»Ò~;?ïûη!ƒ¢?)yö…!]ö?@Å#u‹'?)yö…!]ö?ï¬Q°vÖ?"î®ñZûÃ?"ùër®'?"î®ñZûÃ?ï×Ѽ[÷‰?"r)£÷pV?t!ݲç‹?"r)£÷pV?ê¬Ê£I=-?°Clñƒ?ÅLÕrÛK?°Clñƒ?ïôZ2yO?EU'ç&?WKñ®K1ù?EU'ç&AGN4FGL J0418.2+3807¿ÉL,È,vÀ!ˆr)é–À8ôÅÕaÆÄÀ;mW…!@þ®ð}@ä_á'p?µæÈÌbÏ?Ã11{M(R@SƒãNïQ@
j‡ðú©¿Ó7ØßT¹Á¿äÒ3ß*b¿é¡ÝÀý¿è>°	G§^¿ëØÔ½‡	Ÿ¿ïüøÿZ¾'AGNrdg3FGL J0418.5+3813c3C 111?ïúlPÇSø?BҀ/q•Z?FN½fa¥?BҀ/q•Z?ïìPH‡?gÿϵ]»	?cp¯Ä?â?gÿϵ]»	?ï¯é=àz?/#áàõï?"°xF3?/#áàõï?ïà.A%Ü?V`á¶
`?oÑ⎿›Ã?V`á¶
`?ïÞÇm‰½¦?n¶‹¼ê2?pœIFí?n¶‹¼ê2?ïŸ÷ލ-i?'¼Ø…Ã?ˆNö5»?'¼Ø…Ã?î ±wç? bTs=È?¥ôè'ý­? bTs=È?ï÷îRrW?‡´"#8{?Á2B?‡´"#8{AGN4FGL J0418.4+3414?ß¿"¢ÎemÀ&õû"‰µ À:¶XÆj²üÀ<-+œeü´@¥4°¶Áž@yõÅšç?Ò»ua€ùe?Ê¡õHAe?ö	Œ³?ó9
}‡jB¿Ã>ü•t¿íà
¹(*¿´ZŽýðlu¿àÚ&½+.¿ïÿÜßi‡ƒ?å;
óÊAGNbcu3FGL J0418.2+3412GB6 J0418+3411?ï™ïê"?›?‹^­g?‰"m.*?›?‹^­g?ﱩŸ|,?‰ÿ…LSÂT?ƒ•˜@Âñ?‰ÿ…LSÂT?îzõåþ?š*$òÉ?¨P¡®0?š*$òÉ?ïÌî–Ý8?ƒ¾ë>þ­?œÆb&E!
?ƒ¾ë>þ­?ï‡'Tj?"2Ê
Çí)?Ž8[¤(:?"2Ê
Çí)?ìº]º"â?¿÷*–ŸO?º-r.èî?¿÷*–ŸO?ìÕ÷áðÃ?¦rf's•×?¹Wˆ@'†k?¦rf's•×?éÅC›?³¸¾Vu)8?ÉÀëÞñù"?³¸¾Vu)8AGN4FGL J0420.0+0805¿î)ǁ*ÚAÀ<sz€Ïž8À:¬[y£Z
À<e|[›1@‹¨ÉR9@rT`ªdÃ?Å}
—³f¿"9r½aÊË?Ê·û–ã\@
Ðδ®rð¿ÝN'}ÁKå¿ã:}¿ÉY%¿ëˆ:̄¨q¿áåuoî¥e¿âàØóK½¿ïÿùµc#¼AGNbcuPMN J0419+0804?ïþÓÊíÏ|?Á¶¸w¶?"ÃSÐ?Á¶¸w¶?ï÷®ÈÞ^M?Rª½Øç?P¢mҐ6?Rª½Øç?ïí&A\@?`5â*þ•?bÙ¿'^oø?`5â*þ•?ïÿTdíP·>þÊQSÇå~?sb¡³>þÊQSÇå~?ïþÄ–¢?%Wô&c²#?#¿³Añƒ¡?%Wô&c²#?ïÜùB'ª?}ª©ý$?qƒ}fõºÒ?}ª©ý$?ïÚz5Œe?u£êÝ+Š?rÂå"p ±?u£êÝ+Š?ïü*o—?2úŽÑµ§&?>«õ'ˆ:†?2úŽÑµ§&AGN4FGL J0420.2+4012¿ï™iqøY²Àf'ëØ+À:=k¥jˆ4À<q¾‰=+@!	'Oæ?ýHÊ#¥ ¶?ÃwA)@?¸NÇ~¹ï?ôòôcê‹$@ÒÛðX•?ïë³ýÈî¿ç Çä¡Ö?Ípž"ÀI¿ÞÔna‡"n¿Ú] #÷V
¿à‰äð°AGNbllB3 0416+400?ïüÜ @¬?-ˆu²vù{?9ý×p™j?-ˆu²vù{?ïïÃñ °~?dð$LÍÅ?`<–IA¸?dð$LÍÅ?ïòBîo½[?\9¾Éô:?[z#O?ú0?\9¾Éô:?ïÎb	p¨E?\궱É6x?xÎûFL?\궱É6x?ïùht'*?B˜gÖþ%?J^,Ø×ß¡?B˜gÖþ%?ïŸðö¢´ ?¡6+—?ˆÂI"ˆ3?¡6+—?ïê¾{êöÈ?põÓJ¥¼?eAƒïíoü?põÓJ¥¼?ïnû´ˆµ?~·ZL.u?' ‰uO±p?~·ZL.uAGN4FGL J0420.3-6016?à$—óëäYÀDäÁ¨¬\À:ï¨NhBßÀ<Ҝ¡‹Öb@ãü>Ty@Stÿ†]}?ÀíS*Œˆ¿ŸWÐýD0?ޜš·På@¬ƒ!Ýö@?ïÇËLp¿åvÀ4ü¿å¤)	ä…P¿×",<žìÀ¿Ý@IQë¿á¸I©ƒòAGNbll3FGL J0420.4-60131RXS J042012.8-601446?ïÿ)^Àw?
MG…pô¹?Ú~Ò,À?
MG…pô¹?ï÷ÑGÛ¶Ë?R3?öw¯|?P]p—/àõ?R3?öw¯|?ïûxƒ¾?0'T§K?CžiïìZ?0'T§K?ïþ4=@ʘ?<bϒ]›?,¼*)ðê×?<bϒ]›?ïþÉëà¨?oô䳛?#aA"½7Œ?oô䳛?ïÚ[À	×?ƒ*D¶	/2?rÒ ¨`W?ƒ*D¶	/2?ïû¶Fùc¯?JDÄ»õ4?A&ä¤nau?JDÄ»õ4?ïùÏËk	?92ýé%œ`?HÀѱ!9ž?92ýé%œ`AGN4FGL J0420.3-3745¿~šã*86ÀFŸ}At>–À9?q/EÀ<Õ]•@º–rȟl@b:îéW?­6(ÛìOt?¯
nݝn?þr!+û1@ ³0C"ª¿Ù€ÉS›ˆ‡¿â/2ÝøÄ"¿ãêÅX.•¿âIáf6ì¿år{Gžû¿ç¸W)²€ñAGNbcu3FGL J0420.6-3742NVSS J042025-374443?ïÿ
ÍP³Õ?fh&^W§?FMz~Y?fh&^W§?ï÷ÌÈΙ?Qì:Ϝ¦?Pfn¢¾ù?Qì:Ϝ¦?ï÷ÙK=ô‹?S½ (»ËG?PMiGä(û?S½ (»ËG?ïþ":è'Ø?ÿÉü¦×#?&¼P1mê?ÿÉü¦×#?ïÿ8øDé?ÈPFCë‡?àûä<9°?ÈPFCë‡?ïÝ3z‰f¤?}±¼µ,d
?qfBŸÏÎ?}±¼µ,d
?ïöö+•Úó?X8àp"?R¨¥iê?X8àp"?ïý
øà¿?2I㈝X¾?7¨:Þ+¦˜?2I㈝X¾AGN4FGL J0421.0-0752?æjô ‰ôqÀBsUïÝìÀ:š*
ðƒ‹À<*ºè@ä²hG'@äŠ=Ü¡?Èö¤Œ'É?°o炅¬?娑¹ÑG†?ðõž,Á?ïý
Ú7¿æä¶Ê,	¿å §ªÔT¿êƒÈaƒ'½¿×8À¦MÝ¿ïü÷™Ã
AGNbcuPKS 0418-079?ïÙæèÏ.H?ªë'²†×H?s‹¢ÃÃ?ªë'²†×H?ï¼ÐÃã€?'Ü©L?€ûËðiû?'Ü©L?ï"?<Ķ»®æ? Íi¦?<Ķ»®æ?ï›d˜ÛÚ?q«òí‰äý?‰>¦Ïz5­?q«òí‰äý?ïïÆ£¿?eÖ¶fI,9?`€9?¡‰ˆ?eÖ¶fI,9?î+Ü'ïÄZ?²YഇÇå?­B=ß¡b?²YഇÇå?ï"\"?˜oя£MW?Ÿ<›µÕCÒ?˜oя£MW?ëݸí>SÅ?¬z~VŠ4Ô?À‰K°ì?¬z~VŠ4ÔAGN4FGL J0422.1-0644?î´–­^¦ÀBäâmHÀ8Ïk=e¼À;ØyªæÈ÷@mHS*õL@¬¾9Œ?¦-º<@;ô?´ÿ+Ä©èœ@	†Eÿ¾'@¨=?üoR¿ÒÔÂ$'Q©¿âýÄMc`¿çpÄÜ=ƒ¿ç.³Ý¾n¿éÚ¡oB¿ïÞfÝڑ1AGNfsrq3FGL J0422.1-0642PMN J0422-0643?ïý‡ú­'7?'	Aò]?3À)ÀSW?'	Aò]?ï÷A,?Q
‡œ"Ä?Q}äoàt?Q
‡œ"Ä?ïÙf‹3?wÚáØJ£?s}LšÙþÃ?wÚáØJ£?ïÿ¨·ø2	>ø«2ˆ®Ò?Ò\[{>ø«2ˆ®Ò?ïýyéX§??+^VýÕC?40µJ*±?+^VýÕC?ïÚá·Yaà?tBanÅބ?r$5Âl:?tBanÅބ?ï½G zô¾?ƒLN–ʵ?€®7ÐÄ¢?ƒLN–ʵ?ïÿM3ÿ$Ó?
`½J§l%?Y¼f>]?
`½J§l%AGN4FGL J0422.3+1951?ïÛ=#)®XÀ4œ!ÄuæÀ9òQ~wÕ$À<2¯È@ 5;K/©@m|:
B?¹Ç¿FÒLi?‡ Éû"?ÑÝVlGQ@0fšhÌr?ïÁ¢a¿7¹¿çöÿ.=*¿â Va¶~W¿ÕApx8 ¿çÑ@>ßcӿɤCZÃÆAGNbllMS 0419.3+1943?ïþ?WüÎ?š@ÌH1?,
}4¾Û¹?š@ÌH1?ï÷Weþ»?RPZ°'˜¼?QQ4G|¸°?RPZ°'˜¼?ïõyüg¼t?e:҆Ašw?U‰—¼?e:҆Ašw?ïø=9$"?7ùÅÿqû?Op¿,x?7ùÅÿqû?ïý ³eõ?-ü¶ò‰?6úft9sû?-ü¶ò‰?ïÙY—ÃM?€>'t·?sS48v~	?€>'t·?ïð3n8å?j«ISŠÞl?_™$¦(¸?j«ISŠÞl?ïìòá‰À?Q9nZxâ?c
♈?Q9nZxâAGN4FGL J0422.8+0225¿ïœ'üAY'À?.¢ ©XSÀ:?Ã<*RºÀ;óvñÎäÕ@–7t‹m1@
'¼«ì?ÎÍÉaˆ[.?äN.Km@ Êƒ@¬Lfn¿ÌmÆWߦ¿á(qy‹¿ì!yÍKwοïø˜'˜K;¿ìl5恿ï¦Ñ€ìAGNfsrq1FGL J0422.1+0211PKS 0420+022?ïºtj¶Y?…Êv
'8?båJ˜¹?…Êv
'8?ïs›@àc?•Hù¿°?'Œ—ù<‰¢?•Hù¿°?ìêˆ"_º?¤ØCŸþ<Ð?¸«¾ï-cª?¤ØCŸþ<Ð?îá;%3Úè?ƒÓ
ã5ªi?¡ìM°1í€?ƒÓ
ã5ªi?ï$—Ñ\)?¥½ûå­?›mÝ|¬Ö?¥½ûå­?éŸ.'äM?ÉjîwR®?ɃEôoÂÊ?ÉjîwR®?çAL۝A'?¶5‹2·ô?Ñ}fHÅ|Þ?¶5‹2·ô?ã¡z"ç—?·"&âz°Œ?ؽ
ö0Ñã?·"&âz°ŒAGN4FGL J0423.1+2106?æ¶L:@B»À3§ÑEØQeÀ9É2ÄxjuÀ;鞍õ ©@ŽÅ9°zÝ@#¿!é_?»Jm·hŒ†?³ôÓ|vÕ?ùÝÑ6¾Øî?úO–@HÅ¿Ø¥bïڿهã¤)Àn¿çù‹!0Ò0¿ß8÷b¢Œ‡¿å·a¿ðAGNbcuTXS 0420+210?ïöÝÇÆӏ?EÒǞÝ[?RDp¿P"…?EÒǞÝ[?ïË{?!º ?}üÆ5ï?zB`N&°?}üÆ5ï?ﮂa2 ?'㐹PÀ?"_g¾[?'㐹PÀ?ï \óº¼?~=ÏMk}?›ôa€w?~=ÏMk}?ïàœÒ«€n?e@WŽKÑ?oc-¹~?e@WŽKÑ?î©c(n^-?­Ú%lIu?¥iÍ|‰¹3?­Ú%lIu?ïLùÐ2?–Q{›ø[«?Vi\ÿ¤?–Q{›ø[«?éaòiЏ`?­[QÐÑ@?Êx6X½Â?­[QÐÑ@AGN4FGL J0423.3-0120?ëð\aC¬À@>}QÀ8
g†!ÑÀ;Á%ϝb@•,]@ätÙÆ°S?ÆÅÝÖp¡?¶˜W¾òˆb@ôaùð†@uÏ¢<x¿Ó;ž̬¿àO8añ6¹¿å-F¿×ñÄ¿åâ;Ÿh¿çèµ@i&µ¿ìsüPHAGNFSRQ3FGL J0423.2-0119PKS 0420-01?ïüæ¥2vl?5[ÓĈØ?8ÊÕÛƅ?5[ÓĈØ?ïõŒXµÆ?Xñ3èý?TçNák®?Xñ3èý?ïêcŒD?nœl-{?eœtëû¯?nœl-{?ïÿ"Þ)I-?v!Þx?Èv8ߢ?v!Þx?ïþ"Ñ}?®g-m8?&ρS'«?®g-m8?ïÓP%¢Å?"`±Ãyý?vWíƒüÑY?"`±Ãyý?ïìþ¤œh<?q-3þ"?c[vՓ«?q-3þ"?ïþÁj"Þ?õnt"c¶?#ç掽u»?õnt"c¶AGN4FGL J0423.9+4150¿ëÊ÷nN{À‰äÁ¶UÀ8X-'JTÀ;`e':ØC@¯L$›À»?üƒ3á®Ü!?¥–˜Þ2и?»övÿ»·|@Áv¹Ã@¿úQo¤¿Ì«¥'[¿ÚÓ³¼¨†¿Ú²!$袿ÔïÂ',j¿â"n!EÊå¿ãÛG¹ÒõAGNbll3FGL J0423.8+41504C +41.11?î‡^®Œ?·Z,q»Â?£×Š>`?·Z,q»Â?ãÈÝ\Œ?ÌÂÌߨWß?ØoôEGîè?ÌÂÌߨWß?ìsr'Jž<?§x€sœž¡?¼dku«?§x€sœž¡?顒œzI?£Üõ¾ýd?ÉyµŽً?£Üõ¾ýd?ìPÕ[ä
?¶‡>ÿpû?½yW ß°?¶‡>ÿpû?øx
ûÉ?ÆQMFýü?ëáü<Î?ÆQMFýü?î&ЬÞÎ?¢Í^ y?®}'ñÂw?¢Í^ y?ÑEã#¦M\?±¯ò(+?ç]n,ÙR?±¯ò(+MIXED4FGL J0424.7+0036?׌)ù"À?ÆñVIÀ8«ü†Î»ºÀ;Ý[o'_@Âqû@JTFŸ?§£aÍ/?¬îÄ$÷J@瀕Ó;@S¬½¿œ¿×Õi>!²¿ÚäÑ@±¡¿ä…péP'¿áäø¨ê¿æFV[Vgì¿æÖlÞ¥'KAGNbll3FGL J0424.7+0035PKS 0422+00?ïþ<û‡?`(—|qØ?':maI?`(—|qØ?ïöž§öS¯?Tb:'Ýv?R¯Ü^â¥?Tb:'Ýv?ïî».¿±?pc!ñÂÿ‡?aDÑ$Òµ?pc!ñÂÿ‡?ïô	®™I×?G€«7"S?W좦ð±?G€«7"S?ïý28jc?2¼Â¬Oï?6n=$Q>V?2¼Â¬Oï?ïßAò×s?rQæÅxòé?p_Ù·Žœ?rQæÅxòé?ïèÂò-"s?sС]^?g=
ö7}8?sС]^?ïÞY¿fÍ?eO÷Oá?pÓ~¨‹©´?eO÷OáAGN4FGL J0424.9-5331¿À¦\m
¼¿ÀEÓEŒÒÀ9­ß…65FÀ<A»±–^@Ź'Fî@"
f‹OT?±®xßöÜQ?½U&^Iȇ@
ÚXÁb5@×Õ?7"¿—I›ªjø¿ß,>ø8`¿ã+åï¿ã0AFmD¿ê¤E>Îqè¿ïþú|2€†AGNbll3FGL J0425.0-5331PMN J0425-5331?ïü"OÜ?0Bun<‹Ž??ÃeCŒÇ;?0Bun<‹Ž?ï÷c$ô	?Rô¿Éä.?Q9ÝEd¾ê?Rô¿Éä.?ïÎrÀ֎0?xš(ÁZu?xƟš8G¿?xš(ÁZu?ïü؋Ð`ß?#
=¬Iۄ?9;Ÿò?†è?#
=¬Iۄ?ïùqL;+?DÉrÕAú1?J:̓¶?DÉrÕAú1?ïÙ:´ÿ?'†'hy?sbŠ'"?'†'hy?ïWâÂ#óÈ?óÔ3ډ4?•§²ê?óÔ3ډ4?ïöK¿Ø-å?C'4Ûáá?Sh€4'UÙ?C'4ÛááAGN4FGL J0425.3+6319?ïÐrÊf°@#‰ù&ÇêæÀ9ì
±™kÀ< ÌàîÂÁ@!¹ññIƒØ?ý_ñ7n+?º ³iNx3?"êxg«ò?Ø©ßAÄpˆ@ò`gžÊ±¿Ùž´@cóE¿å®Å"T¹¿ç¼=s(¿Ñ÷†^ÔKÇ¿Ó\ž¼n¿ÚæØ;ÀËbAGNbcu3FGL J0425.2+6319NVSS J042524+632005?ïûÌL§Öý?2ê8wG÷?@ÎÍioÚ?2ê8wG÷?ïï3ŠØò?bӇ"h?`Ìu.ÃFm?bӇ"h?ïìþ™ß Ë?av'Ö\
_?cf
a´ü?av'Ö\
_?ïð08ÏKÐ?G;¯=¿y?_Ÿå¶q¤?G;¯=¿y?ï÷hÖƒ§?C2C"±ƒ?Q.ShEƒT?C2C"±ƒ?ï¦UÖºü?Šî=ÝF?†jŠX 7	?Šî=ÝF?ïäVQx÷?v¡`bd?k©®cLúÞ?v¡`bd?ï¾Ëk½'?p†k"2?€M%>a9?p†k"2AGN4FGL J0426.7+6826¿èˆ€•ìÄ@*º=ú	FÀ9¹ÏµqfÀ<6¸©õ@!lµàÍ
@˜vƒêÛ¬?³¶ûª0?ª´Áp'ý?÷³{?D@yáSígø?ï÷ó¡Íś¿à³ŸÕý¿åŸ+ÿ¸1Š¿à! Ï¨¿ãPW›ÈH¿æ]4Ž}åAGNbcu3FGL J0426.3+68274C +68.05?ïýN¹HÒ?,F¢½^°?5Š2À›¿­?,F¢½^°?ïîsµ¦·Ý?a¨š½Tåƒ?aŒJœ {?a¨š½Tåƒ?ï÷  š¦?B¢ÆÑhí?På¾ßÆóô?B¢ÆÑhí?ïÓë«ùÝ@?Z–òpÛj`?v
)ãtø.?Z–òpÛj`?ïù°¹¬ð ?BÒg/ªä?I=H4¬?BÒg/ªä?ï¨CÝi@û?ê:¾9Y?…ï¢@%B?ê:¾9Y?ïí'F<È?tL|Ö zÍ?bnø¥%t?tL|Ö zÍ?ïZ:@1?|Ò«ú'c?"¸¸AG?|Ò«ú'cAGN4FGL J0427.3-3900¿îÖ¡a[‡ÀE÷—$tSÀ8ä01öóÀ;´bTˆîQ@å†Tmj'@¾–ÃüC³?¨Î½š
L?y~þÈ#n?ʽì(2@xS/'
¿ÝՂ}ô!¥¿åÝÓð­|¥¿êœ¾™XV¿ç8®6Ý¿ïüC²\´?ï|.NÇä0AGNbcu3FGL J0427.3-3900PMN J0427-3900?ïý‰k¶×?0:^gí¹§?3´¢TÞ¬÷?0:^gí¹§?ïøtyQA?SØ*Š(s£?N.H>ö¦?SØ*Š(s£?ïˆûï¾Ù?-®^ٜl?û
?-®^ٜl?ïþEévÚ0?"ŒÔãe?+¡l¼ãÀð?"ŒÔãe?ïü˜rä4Y?=Uà×Úpy?;<fê?=Uà×Úpy?ïà¥å,j?|ü
£Ú?oZí²ñ'?|ü
£Ú?ï~=*¯?á©zñÁ??Hë(?á©zñÁ?ï÷õ™ìòÿ?L=Œ>C‡ì?PÌ1¥~?L=Œ>C‡ìAGN4FGL J0428.6-3756¿×¦\š#œÀEέÙ©TÀ6EXôÛöÀ:©fã@È{zIÈ ?ÿë|Öt+?†Nӑ{׬?´ég,ù³@*Lˆ3?È@ QúÖ `2¿³¢ðŸ(¾¿Ú#¡ZX;*¿â'°âÄ¿áýˆV{7¿åé`F'µ¿è Fý"5AGNbll3FGL J0428.6-3756PKS 0426-380?ïéfÊJ¢¢?gÖ³ºtÝ?f™5¢Ž^?gÖ³ºtÝ?ï³¥.Î?éß6™µ—?ƒ<´\öt?éß6™µ—?þI€?±¡ÏÓOc?¤†0 Ó5ý?±¡ÏÓOc?ïß,a÷…¢?yd]ns–?piÏ}?yd]ns–?ïäÅ1Öok?f>….¥[?k:Íö¶\Ë?f>….¥[?îTË«±ì?¾šÒv&o?§ê³AÕE>?¾šÒv&o?留SÝ ?ŒG%mÄú?†«3)`?ŒG%mÄú?î©ÅšÃ)$?¢ðéæÒÌ/?¥c¦SÍmÃ?¢ðéæÒÌ/AGN4FGL J0428.7-5003?ï<)scFnÀE‡0HAÀ;O¥^ɹóÀ<ˍg\/¬@í
¡~?v@"!4x®?Î×^v-í?¼/'(áö?îŠÒŒ)nŽ?ô†ùç71E?ïþ±ëÕ¿Ò''Û'‡¿èˆ¥@ï«¿ß'£G˜E¿ïÿŽñ ¿îxê݃ÿ)AGNbcuPMN J0428-5005?ïîoNÂZÙ?ÃO…WM?a±,j?ÃO…WM?ï"y÷½¼9?—DAXŠ½?Šá'
!UÚ?—DAXŠ½?ï[br©Î?Ž7™fœUÜ?""±·Ã\S?Ž7™fœUÜ?ïck´$4?v›¤9¦^?"'Ÿ0Z±i?v›¤9¦^?ïüZ¢œ¨?<Ì	õâõ?=*ðƽK%?<Ì	õâõ?íÔzæ|÷?¹Òùó?±\/JI?¹Òùó?ïSÍMð©?5ys.Vó?•†VdÉTß?5ys.Vó?ë=?‡»‡?§ä²sdŽ?Ã"áä?§ä²sdŽAGN4FGL J0429.3-3238?áh$¬ÀEzšu%FÀ;G\WìÀ<иãá¼H@P¦?p?ý™¨bŠ8Ô?ÏN×(›T°?Éó˜Ôw¼?ö1ƒ/ÊÉ@_u†iç¿ïü.ÿò¾ú?ïÿërªAˆ¿Ú#|"jÞ¿åÀ¾/@¿ÒéûF\Û£¿é*°bˆá;AGNbllNVSS J042900-323638?ïü+ê6¢?0Þh¾/Ó?> ¬³Qф?0Þh¾/Ó?ïó4iû-?Yä4~'j?XŗŽþfG?Yä4~'j?ïÁZ4Ì1ê?z!¤ô£Kæ?R宄³?z!¤ô£Kæ?ïó2J¼"?CCI‹œq'?Y›j^€"n?CCI‹œq'?ïøF]/Ü?Hæ«£t"ã?Nå¾€2?Hæ«£t"ã?ïǗ‹CâÐ?ƒó´vvu?|4:<bl?ƒó´vvu?ïW®–gS?6 gBs1?•
-*…¡?6 gBs1?ï 0ŒÆ?rÁñh1Ë?~¯çÈÖdý?rÁñh1ËAGN4FGL J0429.3-4326¿ï¾û¾°]ÀEÅõ@‰]À;å(
eCÀ<¶ýwÞ@bå®pg@ýø8‹?Åê•_£(º?¨ "ûé¬?àÿG¾…ŒF@:~6Ë¿Ú&Gݏ<É?¡9À–¾»¿å§ûâd
Ç¿ìSå1[¿âWÝó»¤?º‹¤ùÜAGNfsrqPKS 0427-435?ïÿvñ?¤Áþ®}?±%f¯6}?¤Áþ®}?ï÷%âxì·?UO
ïè?Q´:¥²r?UO
ïè?ïãJÇÆÊø?m;(K€ãg?lµ8(¶è•?m;(K€ãg?ïý†¶º'?ëo™ˆ?3Ï*,{Ÿ@?ëo™ˆ?ïýôD"?/.+€-?0]áýúŒ?/.+€-?ïÙ¬9s-?'³‡[Ew?sw©Å¹Å¢?'³‡[Ew?ïÇM·Ìh,?açrl?|Y$~VS?açrl?ïðx­³#{?Qž÷¥\&7?_¤?ZÜ?Qž÷¥\&7AGN4FGL J0429.8+2843?êi5úäÀ*óÝüŸù/À9RîؐOnÀ;ÃD°E®@½?Çk9	@` ßs˜~?·‰Hh¤"?¾Ìևá‹K@¢õ:ªú@5PQQ+l?å$Ã9¦¿g¤Ò»VáA¿áhçv¯Š¿ÛuÓáéêj¿äï ×{|x¿è	çàN‰ÑAGNbcu3FGL J0429.8+2843MG2 J042948+2843?ïõÊ8Œ¨3?Q|¹´.¯?TkŽuüiô?Q|¹´.¯?ï¶-ixGB?‰Pè4c2J?'t¥§Å…t?‰Pè4c2J?ïÁE?'9¬ùº—ô?wñûó½e?'9¬ùº—ô?îffb¤SÌ?‡'žžGE'?©™™ÔõI?‡'žžGE'?ïdãkÂV?"îô	¿«Ù?"c'€Þ}H?"îô	¿«Ù?î'>^¾?¬#rÌ«]Ê?¦Ü¿?¬#rÌ«]Ê?îJHÒ=
^?¢'Ƨ	r?«[rÝç("?¢'Ƨ	r?èÝÒ·%#?«£tóHÁÎ?Ï܈µ#ks?«£tóHÁÎAGN4FGL J0429.9-3101?ÚpÃÜÀEIË>WS¤À:&˜Û-¸ À<r$ëqÔ@!uƁ?ýJ½"så«?½¾¦Š˜Ë?»×xÍFD]?þv‰Ê½f@Ô:®0?ËÍ2xMC«¿Þ¦^c™¿Þí,¾¤ëÝ¿ÓPNâf<¿äò?£%¿ç´v)RáAGNbcu3FGL J0430.1-3103MRSS 421-156568?ïþÁÉäe?¶Å¡½iÞ?#ãaö–1?¶Å¡½iÞ?ïöö¯f?R`)&¬?R¡œ¸'?R`)&¬?ïøÝ\š"G?M;Wû/›?LŠ'uä?M;Wû/›?ïð­íí?AW0*Ô?^¤#Ö1ò	?AW0*Ô?ïüê˪&É?1Ⱦ¶±ë?8©¡*©
l?1Ⱦ¶±ë?ïÚ³¬Y(ª?VdVéá#?r¦)Ö+Zù?VdVéá#?ïöM6!>?fÁïIî9?Se"]0cö?fÁïIî9?ïÒ4*Tz?`"KÙô.?våêÆØû?`"KÙô.AGN4FGL J0430.2-0356¿Üˆ¨^óWÀ@}7\ŸÀ:ÖöV3|À<i²?'ÌÎ@'¥e՜Õ@øá…Áu?ÐRVy‰XÚ?º¹»£К?ä¤Váä-@	ÓÆë|5¿ÐbH_bŽ¿æ(ºžÌßA¿è,PÓ¿î,ma,j¿Ð|T¤Çõø¿ïm í¶QAGNbcuPMN J0431-0406?ïÿÈCm'>ùò×ö™Ô>ûöf÷#¸Ò>ùò×ö™Ô?ï÷MB·?QNÏpëûf?QezTD?QNÏpëûf?ïè~3?P?l°´+(íF?gb¦E?l°´+(íF?ïÿ\O]Z?R^äê?v
²jk€?R^äê?ïÿëÂ8™>æHT¯ƒ	 >ä>	i©8@>æHT¯ƒ	 ?ïÜb0n)K?qk¿ÿÒc0?qÎçÕùމ?qk¿ÿÒc0?ïà©¡Nš?vÙspZq?orVd0Æ7?vÙspZq?ïû­™fÿû?9‰£µGØ?AIš€–oS?9‰£µGØAGN4FGL J0430.3-2507¿ë\'YèÀDFÜ]cˆÀ:0%°"±"À<z"UŒúO@wàÎ'.@0ñ¤óið?¹^€hñ;?œf8n0Š6?ã5Õ¿º•"@¬7ñ³â?ïò+
0À¿ãî!	¿â¹·a*½C¿á;w¥S¿ÝXODù"¿ðAGNbll3FGL J0430.2-2508PMN J0430-2507?ïùŽt!ó?<˶"I\n?IÆ0ûý'?<˶"I\n?ïõfŘ`?SÈ[£'µ[?U2t°oÕ?SÈ[£'µ[?ïãl{B/?pW'$¥¾?lÿ"['€Ð?pW'$¥¾?ïîç¸5f?Hÿê·Ùåñ?a÷d§QÅ?Hÿê·Ùåñ?ïïã "õ£?VðˆMÙ2?``&$r?VðˆMÙ2?ïØ:¼òî?ِһI?sóâ"x??ِһI?ï×FtO ?|'àê©h,?t\ŵw·Å?|'àê©h,?ïǴӗþJ?h"7M^?|%–(R.ù?h"7M^AGN4FGL J0430.3+1654¿èÙɂóîWÀ5
ȁäq.À9—ˆŠ}œäÀ;ÉLíï\D@dƒÖcÏ]@Ŝ[cÔ?¶#Ú$ÏU?šƒX ¼3ß?ã¤Ô•îê.@ÆîÍӇý?ïý³õerK¿ƒ]$ԚĿæéu¿Ê°¾¿ãڛ!Y¿ãxê݃ÿ)¿ç}d¿È,AGNbcu3FGL J0430.5+1655MG1 J043022+1655?ïýÐOäï?(—µé÷½n?1}'@*å?(—µé÷½n?ïö½I®j?U<ûß6U?R…mPZk?U<ûß6U?ïã›ð®JÎ?lZp>,³?ld[T÷?lZp>,³?ïð§wJ0È?Fc±pqøV?^±hÞ¿×?Fc±pqøV?ïù‰P´?Eù౧©?IÚà懿?Eù౧©?ï؋ìÕ"S?€7FBÐyF?sº	°;ÊA?€7FBÐyF?﷌èAƒ"?"ZtÍÌm?'Åû¥¼ã?"ZtÍÌm?ïÌå͊ô?f° ~Ö?yú
:6Å×?f° ~ÖAGN4FGL J0431.8+7403¿²íDkEǀ@1^‹\¿ôwÀ9ÿ¦å²vàÀ<oLjÀ-'@ýBÝ ?þë`ºU?´åV 9Šª?¥8iRÿ×;?ð£~õ©e@fuÜ{ ?ïÛS]u&¿×^Ÿ"¦¿ãû–yS¨õ¿ØaéÿãzŽ¿Ö•ǶãV¿èÜ)áû³AGNbll3FGL J0431.6+7403GB6 J0431+7403?ïþÙy•m?ùkz?"o…‰'?ùkz?ïóÇy•‡?_|˜†?Yøp¤`ғ?_|˜†?ïù
fúú¡?>"ɨ¥¨J?KÖe,ì`?>"ɨ¥¨J?ïúS˜')?0Y<ôñùN?F±ù×Ð?0Y<ôñùN?ïþNŒLvs? <S?+9›.>ý? <S?ïÅZã%~À?…¢û[ð/—?}RŽYRäJ?…¢û[ð/—?ïúGŽYÿ?Q²iu—¸??FáÅÈ*;?Q²iu—¸??ïô¢Q#36?DÀ'^4‰…?V»^3É?DÀ'^4‰…AGN4FGL J0432.0+1732¿í5kÈ·$«À4U.ÓÀ:ÆYåN£ÒÀ<pz¼^À@îQ†…j¹@Á]¥Í"ƒ?Ô'øR¸?Ûß©~+V@µ;ÑgfA@"pµßö? S~œÅ¿å(Уñâ0¿ÜÚsÿV6î¿çLê"]ðv¿ï»batE¿ë¥­Aí
AGNbcuTXS 0429+174?ï§0—2È?¯—°ýŒ¨Ý?çò=?¯—°ýŒ¨Ý?ïßqÅȪ?nENvÚ¾?pwÇܚó?nENvÚ¾?îVëї.R?˜>ã´}%?ª'BèDèá?˜>ã´}%?ïx'y±5±?p¤T?ï°ÍHåÐ?p¤T?îù­4Î`B? |Sù×eæ? e,µ­°Ú? |Sù×eæ?ïf²¯Å?™87rë¬w?")ª&‡Û?™87rë¬w?éâöќÚ?²é
Ð:?Èt$¹Œ—í?²é
Ð:?ìHY€NïÒ?¢¿rŸ™^?½½3ýˆn?¢¿rŸ™^AGN4FGL J0433.0+0522¿ÑhžFsúÀ;j¡è´lÀ8ôxmÏç4À;œ=þhP@4@§ºï€@st¼j~ú?²‰`
0ë?Ðý ¿¨¡õ@×õûn@…¤Q¦ù¿×›X¶z{¿ãìÓu]¿éÏ^âäfG¿ìª$Ìh"ÿ¿ð?ëí×^v-AGNRDG3C 120?ïÆv…Ý?Ÿ\šBˆ|?|Ľ%d9x?Ÿ\šBˆ|?ïõƒ²§‡™?T@¾Ò/Wœ?Tøšq·þŒ?T@¾Ò/Wœ?í}é~3b?£Lώä'ù?´ȳ qs?£Lώä'ù?ïüšãÏ%u?,—ÉO]µ?;(áó®\?,—ÉO]µ?ïá܄áâÅ?vypî?n#{5z"?vypî?ïÍ×4?ƒ7[-?ysbùÎ{?ƒ7[-?튛w?Q¥?¤Žä#?³«$D»˜]?¤Žä#?ïÛå2cm?gÔOí85?r
fç0ùb?gÔOí85AGN4FGL J0433.1+3227¿È"°êv´pÀ$åi+<ĬÀ:7®_ú;›À<(<üàÏ@!A¯à+#?ýhò	1?ÂP?§¿!?¥Ùr€-À`?ãn;¢BŠ"@ˆ™úg±?ïìŸ/ۏ޿ê.8!¯}1¿á¥îaG¿؟Úép¿Ö
µ%;Mß¿ç› Yý!AGNbll3FGL J0433.1+3228NVSS J043307+322840?ïý¥?È v?%,¡l?2Ö;Ўï?%,¡l?ïóEÚ!@?Y°=ݼ±?YtKм²*?Y°=ݼ±?ï÷‰wÉ¡Z?\f}U›´?PíI[_?\f}U›´?ïóšëÂõø??Eâ:B?XÊ(׉o"??Eâ:B?ïý0)ž?,©MU™ÿ?7v=>?,©MU™ÿ?ï̆ ‰÷?"ëXãwÝR?y¼°i°œ?"ëXãwÝR?ïï¼=)ùp?uîΗ¹­Ô?`CÂ×fgî?uîΗ¹­Ô?ïÚh5•Ûk?_2ß?rËåD0'4?_2ßAGN4FGL J0433.5-1039?è÷`\C«ÀA²÷üü?À;vºq€vÀ<˜Fíû¾@éEÔJ›@'µÿ_Ç?ÈÒ»y=X¦?®ßM>2{ä?àˆµENJn?ü\±+†–ˆ?ë.-9ôîT?ç­½"4Þ.¿ã&ä¦f&¿ãñV^ÜY]¿ïòbRÛo'?ïGÿ¨Â+‰AGNbcu1RXS J043333.5-104220?ï÷ê€Îç?KHt»å²?P*þ¯M:£?KHt»å²?ïèôñ·›k?uâ/¢<zå?gMãõ?uâ/¢<zå?®jü?'ò¡ÿ‹êC?Žž´?'ò¡ÿ‹êC?ï͂!Wév?c$3Öd,Ó?y>ïiXØå?c$3Öd,Ó?ïð˱2¬>?\æô_õžQ?^hž›p?\æô_õžQ?}V"?'t،LÎ?‰"àÂÙ÷?'t،LÎ?ïg
DkX­?ëB²â!?"·kµ²^?ëB²â!?îÄì`2g(?"ná#	ß?£±9üٍƒ?"ná#	ßAGN4FGL J0433.6-6030?èÜ
¬E1§ÀD5\ÙëÀ9Cº­˜#À<!.b@ݝ^ä'@¨— B•§?¨îL¤Ht8?À³l©v†@:x¯>F@¨Úã:øO¿Ëç*Üw¯¿Üp5½Q.Ç¿æM±>&p¿çÒÌ ×üV¿ê"—8w¿ïýÚV"K"AGNfsrq3FGL J0433.7-6028PKS 0432-606?ïúfæ"ó<?E=n'F¬Ì?Fdf`
+?E=n'F¬Ì?ïö³GŒþÎ?XgÏÃßTÅ?R™p¬Hôj?XgÏÃßTÅ?ïÈÇTÆ^|?wE,è'çS?{œU—Qaè?wE,è'çS?ïýB圖=?"ÛS1?5èÓJ•"O?"ÛS1?ïõïÙ>?Qí1;JO£?T!È;Àbî?Qí1;JO£?ïØñ™ñêO?€:vlòˆO?s‡3ëPž?€:vlòˆO?uVÝ÷?ˆ/"Ir²?ˆÒâŸù®M?ˆ/"Ir²?ïôµ	©€?G#õ ݍ?V•ÇeüQ~?G#õ ݍAGN4FGL J0433.6+2905?äzÓY?²À)3¤r:¯ÿÀ8\iñŽMÀ;9îיå@1ºv^;?ÿ²lHþv"?¨	Ê?eò?¶ÜÝæûw/@e^è¬@»G»ÖZj?ƞÅ''êN¿ÛnÂ@öö¿àobùÊ[Ù¿ßÄ-ÁÚ+¿ä!¸âÓõ¿ãH݉³r‰AGNbll3FGL J0433.6+2905MG2 J043337+2905?ïúrðl?J¬'9Jì?G¦7[£[Í?J¬'9Jì?ïñ…é¹lž?e'ҋú?\ô,4…8?e'ҋú?ïÛ~¢¢?xü"`‹f?r@û›ó<?xü"`‹f?ïù"É?3áêÍQî?K—Î'g»b?3áêÍQî?ïý‰DÚ
?-×Ýõ-±ò?3µØµÞ?-×Ýõ-±ò?ïÃ	{ã?ˆ¯ø×?~{9+Ï¢y?ˆ¯ø×?ïÙ:eEmâ?€¨xóôfi?sbÍsözÑ?€¨xóôfi?ïèÍþó\ü?Wg<õˆ¾?g23£ú?Wg<õˆ¾AGN4FGL J0433.7-5725¿ïӟJMÀDvŽÞT´À:Š:ÏߦÄÀ<š©glö£@_]³d?úBfýe
?Àé(M&#€?ÐC†g­Ó@àÇÀôQv@Sn9œ?ïèC ¾¦ï¿Çq¾ß#fŒ¿Án+ALP'¿Üɘ$y‡¿âw3"«C¿ës,è–VïAGNbcu3FGL J0434.0-5726SUMSS J043344-572613?ïç¥'AL?aº'Úà<?hZÙ	Üû¬?aº'Úà<?ïíœ_¾ùÈ?`²*¡tv?bc +¸P?`²*¡tv?ï~…0xe9?ˆœ2c$Æ?/Y탼é?ˆœ2c$Æ?ïÅÌ«ên?`¨ÑÐÚ?}ªo+';?`¨ÑÐÚ?בּÍ1?™v†ÈpA"?Ÿ
}¡/Sï?™v†ÈpA"?ï 3*
%Ú?"
¸ÏÞÉ?‡ó5lH}?"
¸ÏÞÉ?êU9"5‰û?±¯sCÆ2½?Æ«w)Ø?±¯sCÆ2½?ï-ðèϧ?'Áo†ö?š^éÅC%?'Áo†öAGN4FGL J0434.1-2014¿Þy^ðÀCzÞô¾À:>))ÄõhÀ<"VE†òÎ@&.iIð@4FY€¥?¾£eூº?ÆJL)y@f¨Þ°û@	éaþw¿ª¿ë¦œÒþ¿¼ÍfC½¿áLýpÇ¿éòB<»r1¿Ç^,»C¿ïÿùJYQAGNbll3FGL J0434.0-2010TXS 0431-203?ïû°î¹ ?Xr
í4?Cý;¦Åå?Xr
í4?ïö rü¡Ò?Tª8•=?R¿‹
mi?Tª8•=?ïÎoFù?yÓ¤º¯rÛ?xÿtÍ+÷;?yÓ¤º¯rÛ?ïü©.	å?&PÒçÓu?:³
8«?&PÒçÓu?ï÷Zob8"?Q€Æ]
?QK!m	W?Q€Æ]
?ïÛÜh\q?rûàå¡B¥?rËÈ(—á?rûàå¡B¥?ïMI8G?''´'†¶?–VØð?ÅG?''´'†¶?ïîCx`ö?Vœ™=ŠA?aà¼E¦Šf?Vœ™=ŠAAGN4FGL J0434.4-2342¿ãð*y?êÀCùáuÑ=À:{k*ñERÀ<ˆ]
ô@t/"î;@¼'Æ#?Â8MyZ‰ä?¸IàsȤŸ?óIxÔýó¶?ÿþGn(¨?Õ%‰&"Ï¿ã‡"ØaV¿æ·k;¸<ó¿ã6_mMá4¿æ:®â¬/¿ðAGNbll3FGL J0434.4-2341PMN J0434-2342?ïú¹Ââp×?6Šoè|Y•?Eôd¥U?6Šoè|Y•?ïíù¥uà?d\È<"?b~˜c?d\È<"?ïàw1ë«?n{3+îFÍ?oˆÏÏ‹?n{3+îFÍ?ïÐãX0©?[1Èo[?wŽT‡3@?[1Èo[?ïøû@Ÿú©?C¹*c©uÔ?LýˆTks?C¹*c©uÔ?ï·Jq¾3W?‡©B°Œ?'-c…tjS?‡©B°Œ?ïÊ9Gl?{õ;38bÜ?zãqsœš)?{õ;38bÜ?îÚ.œm?‰whg( a?¢]7x2?‰whg( aAGN4FGL J0434.7+0922? ‰KœVÀ8ñ|å-íÀ9—b=⹞À<ˆv[¦ð@ RGS?þ9¬CÀI1?¶¤u7d›?­-rð³*?ös?wåë@0»O÷º?îÄâÞ0¿ä/P…S'x¿Ø,¹¼¤¶ƒ¿Þ0{rçÿ¿Þ\ÐERD›¿áÜP=Z(•AGNbll3FGL J0434.6+0921TXS 0431+092?ïþ÷¶t4Ÿ?\ü>y­è? "˜)`iè?\ü>y­è?ï÷ý	Å?Tüþå¦?QÒPÞ¶ ?Tüþå¦?ïøˆ®A?>"æmˆ?MùßÊÁ\ê?>"æmˆ?ïú0¾ljj?0"'T
¹Ë?G=N†B?0"'T
¹Ë?ïþŠˆôI­?ÑÍìÃiš?'Wp;Ú¨?ÑÍìÃiš?ïßØé?taWi6?pòï¬æÊ?taWi6?ïù _=t¢?Y²KmAñð?K~ƒµ&Ó´?Y²KmAñð?ïô™Åcvó?DbP''xZ?VÌtü˜ú³?DbP''xZAGN4FGL J0435.4-2623?êßÇÓóvÀD6ä:§›»À;OÞÉN"À<³fZOØ@¼{päš@!G®zá?Ê-ªɏV¿'³Í;Kta?Åû€ÿÄÆÄ@xsŒ>½*?ë¸[#*?îì1¡¸¡ó¿àµpà<ì¿æû½¥h¿Û¯ùWoRž¿åQ‹
ÜAGNbcu1RXS J043518.7-262120?ïü¼S$a¬?6,¯»åãæ?:e–d'"?6,¯»åãæ?ïõűz?W aåZ[?UÆuÁâ[Õ?W aåZ[?ïßòzA Å?o¿ÆX,O‰?pÂʑõf?o¿ÆX,O‰?ï÷Uêö·
?8ò ¦¤»¼?QT)ùÔ¼ã?8ò ¦¤»¼?ï÷¹Nã	r?NÓ¯¿[)?Pb†ä\u?NÓ¯¿[)?ïÐJ!P ™?"«2èÇj?wÚïn–?"«2èÇj?ォ»@n–?'hÿuþù2?€•?¢Y?'hÿuþù2?ïÚ=zM½½?djH`P~œ?ráB¾T-¼?djH`P~œAGN4FGL J0436.2-0038¿Î)Ö'¿aªÀ>›Ã?…QÀ;«ÆÂǐÀ<¤Zk†`Ø@¯}óJå×?þ"þ)f*×?ÒZžý0ÂÁ?Üÿf<Ÿîr@êf}ãZ®@'§Dýàì?É»…õLô?܉uʇx/?Ë| 7 ¿ä',ëp¿æÌÁd8å¿ïöBmbÚAGNbcuNVSS J043614-003637?ïýÂPO¬?2Fh´µz&?7ùìã"»?2Fh´µz&?ïðLþ­¼ß?]+«šò
ÿ?_f""ø?]+«šò
ÿ?ï•JÑËo?~ó2ݺë*?Š­KÊ{0D?~ó2ݺë*?ï üÓy‹?hûùþæ§Î?‡ÀËBÑ9X?hûùþæ§Î?ïû'+p¥?@'˜™|Âs?C"cNñ^?@'˜™|Âs?ïÂYïé+?‰›M.0?~ÓRN?‰›M.0?ï9‰©êþ?•Z8™7?˜ÎÊÉtÜ?•Z8™7?îç|ïrqÀ?‰GŒ¸è~?¡ˆ1Hú?‰GŒ¸è~AGN4FGL J0436.7-7148?¼"éñºGÀAûÇ£˜ À:ÇĹ­À<‰‡¿}@ð¥¦Ã"Õ@úR¹á7¾?Ä1?¾
†?¡J=CŠø?ÜYÀ@Lv@¬ó±³?ïö!úü‹¿ãë½RÜF¿åòCŸ'Æ¿Û ë™á¿é\,9
ä¿ähF&*AGNbcuPKS 0437-719?ï~ÎÄQº?¿W
?&<uȸ?¿W
?ïô[Õqi­?Y
ð&,?WHU	îՄ?Y
ð&,?ïã HŠ]g?j%¶J
Ú^?l_·°»á ?j%¶J
Ú^?ïñq³æ:Ì?A¾:uìýâ?]˜·{g¹?A¾:uìýâ?ïÖøə«Q?wtvðÊ?tƒ›E¸;[?wtvðÊ?ïÖI.-v?~&r\H=L?tÛhÆèÝ$?~&r\H=L?ïÔgxº?|†Z#¶?uÌCûƒt¹?|†Z#¶?ï¿OìÒQ?hóh»ë}?€8ìI‹¸?hóh»ë}AGN4FGL J0436.8-5223¿ì;_&¬ÀDºëp&ÉÀ;x¶ËÈÀ<¤FvÜÖ@+}‹Q@Þ0å{|?Á҅ÉX#-¿³­FàH?ðÆB‰èK®@
¬Tš.‡¿åCªåx,¿ë‡—Ù¥ù#¿å>™=~:ÿãx^Kò¿ïy4i"P¿ïúâm©QAGNbcuAT20G J043652-521639?ïþ.Û¤oÐ?$^óàŸØò?-Hzåëú?$^óàŸØò?ï÷t´N?R:ñç80è?Q؄&ÿ?R:ñç80è?ïä$AJD"?pÕÓÌe\È?kÛ¾±›ãà?pÕÓÌe\È?ïþ;¯?Hçæö¡T?,O» É??Hçæö¡T?ïÿ#w1ƒ?¿J¡ù¬?'ÉõÆ?¿J¡ù¬?ïÙâΰ–z?u{b5M?s˜«$^ï?u{b5M?ïî+Qg{º?l"gkƍô?aÔ®{§ò?l"gkƍô?ïðª¼F\?T¥e›Ý?^«ôš±ª?T¥e›ÝAGN4FGL J0437.2-5846¿¸|8`0ѶÀDØ@žUÁÀ;:†—DÀ<—7£|g@ûy¹h@`V#ùŒ?ÇÝÌ#""z¿š¡éŸ@x?Ñõ몦?ý›Eìu?áŒwr¿ét ά Ý¿ìx¨B~՞¿È§ùÈ-¿éoîo´Ã¿ïü–ž½oãAGNbcuPKS 0435-587?ïøâè+?D9Dï(Áû?Lt_ô°Ò›?D9Dï(Áû?ïì–b¿?n»ì¹×?cè÷…!8?n»ì¹×?ïÁÏCùÞ?sÕèÂ[5¯?{ÐD¡Q?sÕèÂ[5¯?ïòsjäX?B2ßÿf?[*]ˇ?B2ßÿf?ïñM:ƒ?ZWYIJr?]e‹säV?ZWYIJr?ï¼~Ռӧ?'ÿ>ڞV?€àJ‹õE?'ÿ>ڞV?ïÔIL?ˆX ¤&›?ŒŠùxu?ˆX ¤&›?ïHêÔí?¸"ƒr¢?­ùÅJÄÂ?¸"ƒr¢AGN4FGL J0437.4-6155¿äþ@ątÀC§´ÃÁ‹PÀ:ÄC͵*À<¿	A=@ŠŠ}òÊ@>aÝj©Â?ĕpªä?¸± Hõ½1?òÊɽMÓÈ?ý÷børÿîWZ$8Äm?ȵ˜¾'m'¿âJ¹—e⳿ä5V#"Cø¿à| 9›Ø¿ïþb¦¾EKAGNbcuPMN J0437-6157?ïü
Úpñ§?4N:ÇQÖ*??©,)H"q?4N:ÇQÖ*?ïʎ?b6 Æo ­?aVk+Ó§?b6 Æo ­?ïâ?˜Ïͼ?aHò	䯓?mÀg"sÔU?aHò	䯓?ïåÿE<l?PxU©Ž/?jºù‰	?PxU©Ž/?ïõ€bïl?Nš×ÿæÓ6?Tÿ:DãÌ{?Nš×ÿæÓ6?ï¶Y{Ïâ´?Œs¨|"ä?'i ýAø?Œs¨|"ä?ïÅ2Jï¬:?€R74""B?}fÚ}Û??€R74""B?ïX[ð°p?ƒŸj–²@¨?"ôðÑ&?ƒŸj–²@¨AGN4FGL J0438.4-1254¿èH'™šñ3ÀA£.3ðÀ:‡;ibš)À<^÷ÇLZL@»Ç<êìó@.O[‡æ?ÃÕgûè?¦ÏÆÁã?ävÓ xñX@p¾µ²ÔÔ?Éص¹4êm¿ä¨¿¨!¿èqÐý³õe¿Üv<eç¿ìÊkÞöE¿ïÿûÎBÓAGNfsrq3FGL J0438.3-1258PKS 0436-129?ïüÃÛó—?.†Dª°Œ­?;âµÛ?.†Dª°Œ­?ï÷ÓÈáÓ?Q뉞u[­?PXn³*Ò?Q뉞u[­?ïìRÅäj?cŸ²ÎG?c­9ç[ß?cŸ²ÎG?ïý;p«?[…Lޒ‹?6$}ÉÙê'?[…Lޒ‹?ïýû…O,?'Ø=`WT°?0'B¡© /?'Ø=`WT°?ï×ù¥@c?( Ö%?t-LJ"?( Ö%?ïôx×1?e!¿™c¸ê?Wùô(€…?e!¿™c¸ê?ï÷\!
‰?A'ÉaQ…?QéGeôîU?A'ÉaQ…AGN4FGL J0438.7-3441¿â€úŸÕ8ÀD¦^5?|îÀ;"xt…äÀ<ãJ?¿2°@!(dC '?ûë÷j/HÃ?̈éH-–;?ºPÓZ?ð¦<åd@›‹9¬³¿ïù_‰X?ïúµ´)h?Ù®åRп½ÕçRµ­¿ïÿÐÐgŒ?ïÿ	àÔk¨AGNbcuSUMSS J043612-342230?ïüŸ~Ç'?B%öÔôÆ?;Þ2É?B%öÔôÆ?ïöÇïÔu?TŽš'
Óa?Rào™¦fÕ?TŽš'
Óa?ïKÇC éš?A¦~ßx?–‡Rhº?A¦~ßx?ïõ^®XÛ?F›''ŠJ?UB¢àìɪ?F›''ŠJ?ïý!wã«$?7ã3øON?6ô?4¾%?7ã3øON?ïØèl­?sÿ'xÎù?s‹Ê-ik?sÿ'xÎù?ï"ð€8Ó?‹¤äkóð²?ŠÃßî[ Œ?‹¤äkóð²?ïâ0-3-Ä?h®Ô—?mÏÒÃ3Tl?h®Ô—AGN4FGL J0438.9-4521?ì.â'&òÀDâ$ p¹À9N¾7ޓŸÀ<Nªaâs@¨ªÙ‡ñ@c¤G?¬™šròç?¯­Hß(*R?ÿ —Œ™@/&3E|·?ïþŽäÒ}¿ãþdßӏµ¿å}U¡E¿ç0§g¸uþ¿ç­ý~ÆY–¿Ù³œÅH'AGNbll3FGL J0438.8-4519PKS 0437-454?ïþð&VÞ?$;òO|‡? ý˜$õM?$;òO|‡?ïöA/»P?S_ˆ>9þ?S}¡è†àY?S_ˆ>9þ?ïði¡¦¥¾?^oy¯¡G?_,¼È²È?^oy¯¡G?ïìd´#wm?Rˆe‹h]?c›L	ãjˆ?Rˆe‹h]?ïþ­
c§? lY÷ÞÝÛ?%/aɝš? lY÷ÞÝÛ?ïÓÉ¿éø?ƒ–:½?v c> ?ƒ–:½?ïÝÀ3ž-?s9¢w?qæTÔ1â?s9¢w?ïµÌE›ô?sèˆE°w¥?'Œî¦isP?sèˆE°w¥AGN4FGL J0439.2+2151?وæ0ԑÆÀ0KL<µÀ:V3sÊÒøÀ;íK¿3@çښ?ܺ@¬Ì¤ˆàå?ÑÈ3'˜?à¥e¶™…@ql¤nò@X¶ÄLˋ?ïþ8µS3"¿ã¹]¯2³¿á6,!qé¿éò3¿ïúÝ¡†M¿ïÿR@>´qAGNbcuIERS B0435+217?ïàÐfy•?pVc+£èÂ?o/™¸ZÊ[?pVc+£èÂ?卵G"W?ŽÐWËâÐ?†ØÜ `zm?ŽÐWËâÐ?í~s^$+6? :g÷3sb?´eÞ¦O? :g÷3sb?íõ%…ͽ?ò;DšPÞ?°V×¢Ä?ò;DšPÞ?ïo·óÌÀã?'2•Äñã½?'	Žþéˆ?'2•Äñã½?î‡	=㲺?°»Ù$ª÷h?§l%4p_?°»Ù$ª÷h?êY‰:?°´?°1i:0qp?ƙÛ=1?°1i:0qp?äëÏ¡¾V<?°Ä5‡Góº?Ö(`¼ƒS‡?°Ä5‡GóºAGN4FGL J0439.4-3202?éH@AtОÀD_鞔«À:}WƒÀ<†"¢¹ÓÌ@ßeSÁÉ?þò?¸|³°?¼ÂSw rç?6¨ÈO~?Æh®ª¢ÖY@±÷ò"ò¿å@XëS '¿ÖByaÀºE¿ãÜ'"€{¿Ý k…˱¿ÎÌû›Â=ӿ䔦 h?ÚAGNbcu3FGL J0439.6-31591RXS J043931.4-320045?ïþX 0)Ç?Õ˨H?*}øÅ«"'?Õ˨H?ï÷ÿ d­?Rp³<r?P¿}'?Rp³<r?ïùB¢?8IƊ³d?K‡ôŒ¸?8IƊ³d?ïþ¬ª‡Al?q"@'g?%5Y‡â®u?q"@'g?ïý7$s@®?*àæ_õ‡?6FÜÇÕÔ8?*àæ_õ‡?ïàõþõ>?pÀÊyÐo?o
C'"?pÀÊyÐo?ïú6—€»?]/²¼µ8?G'™M¦4?]/²¼µ8?ïû³zÉÓQ?40†pÔÕ?A2ýXz±?40†pÔÕAGN4FGL J0439.8-1859¿ï'Ø
Xê8ÀB¢\þޗÐÀ:
lâ˜À<L›ó-u@؉À]¨¨?ü*î «†?»"(k"Œ?¾Íç©òØ$@}¢™ó\@?'˜rÓ?ìÓ}c.¿¨Ç(H¦¿àÿV"tn¿Óeî[è´	¿ãó·‡Á*¿ßqoC"ºAGNbll3FGL J0439.9-18591SXPS J043949.5-190102?ïý™ec©j?)Þd즳ü?34Ó/L˜&?)Þd즳ü?ïóՒ÷œ?UZ-sWÈ?XTÚy;â?UZ-sWÈ?ï黆'?vÍ®à€%?fDÿ¥õ?vÍ®à€%?ïÑàé
ì?VûdjXÓr?w‹Œ†MÇ?VûdjXÓr?ïñ£"9ûq?Y˽2ÿÔ?\¸ÙUï?Y˽2ÿÔ?ïÔ #!?}Çõú"z?u÷¦ÿsÁ?}Çõú"z?ï¶(¦<j??ˆÑüÀ
)?'uÖ}DL?ˆÑüÀ
)?ï`õäKj?z²å™Bì?"áCuwZ½?z²å™BìAGN4FGL J0440.2-2458¿Úr€&Å«ÀC‡+À:ªá»qZ¶À<q¯x(/Ê@!²§'h˜?÷<Æúû´A?Æ-—<òú‰?ÆêÚÿÀj@_l&™Ç½@ßDd¢¿ïý;)¡¹ú?ïý¯žÐ?݃¾š?¿ö+ëÁ.´¿àÏìÝ
Œ°¿Ê¢Âiq‰AGNbll3FGL J0440.3-2500RBS 0570?ïü›kÃ9?1ݐŽ
Û?;$¨È·ò|?1ݐŽ
Û?ïòF½dá?Z%Š3Ž7'?[r…-þÍD?Z%Š3Ž7'?ïܬúžº?tàÜ
±hH?q©°ã;f?tàÜ
±hH?ïÓ,â%x?`Q25?viŽõµÓÿ?`Q25?ïó­ßvȉ?Q=¦1¸æ?X¤@žü?Q=¦1¸æ?ïЙK§."?}ÄÁ+¥V?w³ZLµ	ì?}ÄÁ+¥V?ïÀ12ýÙ4?‹æ¤?çf'AqÌ?‹æ¤?ï‡áï¯áì?fC}nšÜ?Ž"æ½?fC}nšÜAGN4FGL J0440.3-4333¿ï/"àCøÀDÆÙßÚƋÀ9¤*ߧšäÀ;åíùm@¦'€x`d@³õ€J=;?¹»æàõ"×?Úù\ã/å¡@C!°9ï@Â=Л
¿åEÄe>Š¿ÖNØ²´¿è™'6É?¿íM%'pˆ(¿ïÿ‰b"ʨ¿ç€VÂYQAGNfsrqPKS 0438-43?ïöcãÄ?¡,¬Tˆù?œ_á6ó#|?¡,¬Tˆù?ïó4°`Ûb?h-­ãr?Y–Ÿ8ÉÛæ?h-­ãr?æÊ*/£?±Å:ù€M?Òkªåé º?±Å:ù€M?ïý8Íw?.<ò{œ.*?69—­ÿì?.<ò{œ.*?ï2
ȄW'?›õ.3Ò¼ç?™¾Fø¸?›õ.3Ò¼ç?ïÓ^6=?€õüÉ¥2"?vuP×æ]Ñ?€õüÉ¥2"?êYÜüV?¯˜}èG®i?Ç昌§Ê?¯˜}èG®i?ïéCNoŠä?_Ëþ§Uö?f¼±ÇnÜ/?_Ëþ§UöAGN4FGL J0440.4+1440?àÞv,y}À4~=jΫÀ9ߨ‡s&À;³\ÜJ@;2ú(P@ÿV"tn?ÈÖMªñ?Æø´FÄ	°@;{Q^—?ýig…d?ï^"ð•(ò¿ä´ÔÞi,i¿Þù‰ƒÌÓ®¿å†D
K¿êGq®™¿ïþaAGNbcu3FGL J0440.3+1444TXS 0437+145?ï¢(¾æ?ƒmK'7–?‡uû»¿â˜?ƒmK'7–?ï{ą«{?OlSì?Ÿ‡hkX¦?OlSì?ï
m¦Ìˆ?'öC¹tG©?Ÿ>RDG7	?'öC¹tG©?íÉU4¡«?Špߋø8?±µV\¯¸¨?Špߋø8?ê%käˆ?Àa˜I@}?NjjPoá?Àa˜I@}?ì۔"þؖ?¼O}ÛfÝI?¹#[aSÌ?¼O}ÛfÝI?çÒ6Ä
?¶õ½Iá›G?Ð["Àwåü?¶õ½Iá›G?ãÍo>Ò"Í?­3`Tf?Øe!'[ºf?­3`TfAGN4FGL J0440.8+2749¿ï7ì.֛òÀ(n~¥øL­À9x
†Ñ?ùÀ;éò‰õ·¨@ $~Pg÷`?ÿU0cu^?¸ÞÎWˆ?¸ç÷±¡@Ⱥáè½Ä@6ù8¶¿æ£ùdo¿àTl~Xu¿ã…‡"ݘ¿ÚÀWVP¿Ù²¾c}}Ú¿ëÃßóðþAGNbll3FGL J0440.8+2751B2 0437+27B?ïúp膢Ø?9dD`c#?F<^SôÛÔ?9dD`c#?ïæB±¢Ç7?grÈ#º®?i½N*^'?grÈ#º®?ïÑi³¼ŸG?yž'fi?wK&	£©?yž'fi?ï¢òÌn`¹?iWT7S@&?‡CLç×m¤?iWT7S@&?ïëý9Q/s?\@êN½{??dƉ´Åª?\@êN½{??ïŠqy{'O?"#ôV¤ù?c¡¡6,H?"#ôV¤ù?ïQ_Õ8è?ðN˜O¨Æ?Ô8ï?ðN˜O¨Æ?í£'Óú
?›Ú"öď?²ãi^wáa?›Ú"öďAGN4FGL J0441.3-2617?îÚôœŽZeÀCÅ'U°6À;ù>U¦$ÂÀ<ý/iz@"_Ë1í
	?ø…ÇŠm¬¬?×ýÍáéO?Ân³|n»u?êG-ñªÒ§@|±¬_ð?ïÅF%~>Ê¿ïç7a–
?èìcÔ¿àùþ"ï6¿˜¨[ÜÓ2Ë¿Ò`UÀ¦Î¶AGNbcu1RXS J044120.5-261659?ïþ¾"©¼ì?$Äö4?$ԗ®å¤?$Äö4?ï÷÷e–w?Q½.:?Qþ—Ã?Q½.:?ïñ/.äƒ?T®{1?]¡¢!ÊÕ?T®{1?ïý$"¢ó?&¡Ò,f=T?6ÛasG¼é?&¡Ò,f=T?ïýüA{í¯?)®'f‹,²?0ôò"Cí?)®'f‹,²?ïض"$×?!2óÑØ'?s¤½èÅ(?!2óÑØ'?ïåïõ/'?q{ÂJÀ&!?j
èÒîû?q{ÂJÀ&!?ïøäx0J?E˜y¶µÁ;?Ln¶j7Ç?E˜y¶µÁ;AGN4FGL J0441.5+1505?åkj°‰0|À4	ü›ÇqÀ:RžŸ'×ÞÀ;ð³£¼@!ÔE¼ø™@<êòQÁ"?Á™#RŸÊ?vX\ÇÝù?¸]†Ð&?ýòº‡¥Ñ5?î]'"ƒ¹¿ÚF\»lӿ七Ÿ\Q:¿ã—d53¾s¿×ü}"€U%¿àìm|]]AGNbll1RXS J044127.8+150455?ïû#v@'Ü?4Hš¾ÿÄ?Cr&ÚŠ5?4Hš¾ÿÄ?ïò¯íÃèM?Yè Ñ3÷B?Z $™+¦r?Yè Ñ3÷B?ïç&Ñ겫?c¥¾ùùùO?hÙ.4é½.?c¥¾ùùùO?ïá]p§¬?ReeãqBz?n¢a/c|?ReeãqBz?ïõv¡ii?LNôlUÜ?U½*nÍ?LNôlUÜ?ï×1T`Õ?t­IŸê?F?tsgAáÙp?t­IŸê?F?ïз]Nå–?~®Ü#e`†?w¤QL.œî?~®Ü#e`†?ïc$D$iŽ?€ø'x	åÔ?"›w~âj5?€ø'x	åÔAGN4FGL J0442.6-0017¿èu#:;À<v\=îxÀ7æ#ú±À;¦$p!Ñ@4{;4´h@ßýç!é?•@†Êñ?±¯=oÍ@ÃÀ;ÄÒ-@¢…pµȿÓc?ò©€¿ãYø™Ú¿æ\Ëè¡>ª¿æ••"z›¨¿ê¡Ù¿#–Þ¿ïþš¥2TAGNfsrq3FGL J0442.6-0017PKS 0440-00?ïøВ:eé?F©Â®Ix?L½¸‹ì?F©Â®Ix?ïøoÐ-¼?P~íííýt?Oº@rQÒ>?P~íííýt?ïÆîfzˆ\?}$¡ñ¿ú?|ˆÌ¤Aý?}$¡ñ¿ú?ïÿr5zT?I£ҌÂ?¹X†ˆŒª?I£ҌÂ?ïüP,µ
?6 »Ön´?=~›ë'Òå?6 »Ön´?ïÓù]4ʞ?"ŠêTG*?vQ}§ôÇ?"ŠêTG*?ïãùïÅ 3?utv^ÖÀ?l$bMd?utv^ÖÀ?ïþðð\bÆ?j.|Õr? ðýüÿ°ç?j.|ÕrAGN4FGL J0442.7+6142¿éë¢i»Ÿ@$^°ËæÀ:2"ѼsÀ<:ÏߦÄ%@ ö}¼ÄA?ÿÀ©"£˜÷?¸F x[Š¿u-¤Òîá?¾¢8FîQ?ú"êpvµ"?âÈ9À.¿®¾NÀézê¿çf>ù:!¿ØïõÆÁ¿Ý"F¡$'}¿Ö¨À(#¶AGNbllGB6 J0442+6140?ïùÁ©qí?:÷«Ðýxÿ?HùZ¾ú;š?:÷«Ðýxÿ?ïç^ßð|;?iB6¿«6?h¡í'­?iB6¿«6?ïë·'bß7?d¡Aô	.T?dHؤÕ?d¡Aô	.T?ï²9›8?iìsÕë}?ƒ{q²Â,?iìsÕë}?ïóÒÜA›?P[ŒŸá^?XZGqËÇ?P[ŒŸá^?ïqå­eË®?–UŽ'x™â?'ÃJN @?–UŽ'x™â?ïåN÷'{Ì?tmÂu
ç
?j±q£¼I?tmÂu
ç
?î¥ì(1ÍX?ŽhÝT¨z'?¥¡=~šø…?ŽhÝT¨z'AGN4FGL J0443.3-6652¿ÆŒ›l¶WÀBš-û¹À:@èþ[»À<t>ÿðÈ@û>¥,J@'Œ¢:R?½PÓs?¼f7íW1?ü°qgKh´@
ëc€­åV?ïúŸmîðä¿æ¸à0×¹¿äƒ`½Z¿æ=ø=éŁ¿èè®	"&¹¿ïÿÿ&¦³AGNbcuPMN J0443-6651?ïüá‰êœc?L)Ë,C?8ó°êâtü?L)Ë,C?ïö†ò€™?Y  ÷€Ü?SÊò{3Ý:?Y  ÷€Ü?ïë_ä¹tù?Xn
bº?d "Ï•?Xn
bº?ïùgh!°?3ƒ´6Ê2¼?Jb_=É2?3ƒ´6Ê2¼?ïø"´,—ä?Dñz™g?M­/Ú‡?Dñz™g?ï܂¦§¸Û?}ëö4Ütð?q¾¬¼¡²s?}ëö4Ütð?ïμY?¿ç?{ȅ·YÞò?x¡ÓJ"Œ•?{ȅ·YÞò?ïëb"B]?RŽZõ¾?dÞ{?RŽZõ¾AGN4FGL J0443.4-4152?ÙÉjF¼¬ÀD{BB…À:ôG1ùAÀ<±æõlÿ@ €ö|²Ã?û…‹Z;µ¹?Ènþ"n\?¿"xuœ9?öÑPüDŠ@'°f·š?â=Œ²­è?Üæ´yý¿â©ö©L¿ÀÉljÁà5¿ã»aÕÝ퇿ߪÛá<ÆZAGNbll1RXS J044328.4-415151?ïþL>Ð}å?Ù4CE"?+<Åí/"?Ù4CE"?ïô%¶?V
«¤¼Ý?WµöÂ?V
«¤¼Ý?ïówtß.?I¬/¾Ÿ?Yá³Lå3?I¬/¾Ÿ?ïèy9üi?Hj}ÃB?g†Æ~b/B?Hj}ÃB?ïúÆQ??ß>^PEW?DçµçgTß??ß>^PEW?ïÑöÒÚ­á?€Äó‡õù?w–—xƒ}?€Äó‡õù?ïôÉ}âÙÔ?]xTžì€y?VmS	†ù?]xTžì€y?ï¯",>Å?k¸ÛÙþ	@?" ¦ÜÃ?k¸ÛÙþ	@AGN4FGL J0444.5+0719¿Ðù·Ç,#õÀ7ô§Å¬GÀ:W«(7V®À<"O¶
é@¼R˜©.¸@yŸâÚU?ÂVy^e»ò¿›àûF̆ñ?×>;"»f@	úõÕÓ¿¿þëWýB¿çÒ(¡‰Òý¿ëeHŸ5Û¿ÕñŠ;­«¿ïÿñAÌ(7?ïý ¿¨¡õAGNbcuPMN J0444+0717?ïü¤rÝåp?4ÿMþ«ÿ?:ÜhßZ¤?4ÿMþ«ÿ?ï÷ºÔG5?Q;BÙ;îŠ?PŠX6ätß?Q;BÙ;îŠ?ïç"øש?g,aˆ2Jt?hlðÅÿ	?g,aˆ2Jt?ïþå€ö?b~BF)&?.­ò5'?b~BF)&?ïýnjÁ¿Ó?5™‹bZ?4Œª
~D‰?5™‹bZ?ïÚÿ¨Ê?~ÿºÜû$?r€+¼JäJ?~ÿºÜû$?ïáLÏ1ñ?r1'Šöx?n³€mG.ÿ?r1'Šöx?ïñ'ÅÑD?T*Ô ›ãk?\Út:ˆ?T*Ô ›ãkAGN4FGL J0444.6+3425¿¸ÆO±ÎWÀmtO]5eÀ9Ÿ¤¦=À;¸Ï-Ðã@à²;Qæ@™ÐcZBl?¼5ŽäÒ?­ê4"ö?óÙ&­ó"@M£ÔfÊ¿»j^˜'±Ä¿Ò£®Zñ¾¿å^ü_ag¿Ü^î7€ŸÎ¿è,	æ~O¿ä»ÁŒ§ÄAGNbcu3FGL J0444.5+3425B2 0441+34?ïýçO6?!fàUàó#?0ùÿnv?!fàUàó#?ïñGí÷·)?_†˜Ï³ö¬?]p$yÎ??_†˜Ï³ö¬?ïä·¹"	~?xðz&üµ?kHFQ[Yó?xðz&üµ?ïé9ÌÌÄ6?Lf»txÿ?fÆ3hÕ±ï?Lf»txÿ?ïõ¨Ipón?TÚ@'™?T¯l—ht?TÚ@'™?ïµb\|€?ÀùŠ5®?'§iwåâ?ÀùŠ5®?ïԋT~Ô¿?€P[ÿ"€ë?uºUÞÒ0€?€P[ÿ"€ë?ï›ó0cË?s$
ôõj?‰3ñ\Ë?s$
ôõjAGN4FGL J0445.1-6012?ï"©LPLÀClX£/D'À:£ó}:¾BÀ<®þs8@ìVò8Â?ÿFŽ¾?Âæ¹G‰×Z?¸`ÏΉæH?õ>.‰€Fâ@	lY夊?ï›h zÉË¿êÑùÝQ)h¿ÙJM@¥Œ—¿ß£ü>Ty¿àŠÕ±wÝ¿çÕøÅyAGNfsrq3FGL J0444.6-6012PMN J0444-6014?ïÿ!3èv?8ju*t?نÿ/†S?8ju*t?ï÷"ÀÑ´?S2H¦Þ¸Ê?PØŽ¥§ž?S2H¦Þ¸Ê?ïúðS1!Ø?4#ñYÖR?D>²ô¾Ò?4#ñYÖR?ïý+I·?Ñm{³?7î¨|Û¯†?Ñm{³?ïÿC騔x?
Øs9*r?'ÐË_Ð?
Øs9*r?ïÞÈkz]¥?p`AˇÁk?p›Ê@}U?p`AˇÁk?ïüxÃØ~Ô?H*¡ÏvU)?<9àw9Z?H*¡ÏvU)?ïøÀ]ӚÇ?;#Ö,öô?Lþˆœ°Ü²?;#Ö,öôAGN4FGL J0447.2-2539?ê4z8³ÙÀBÖ5"_õÀ:ØøúRAÀ<¨!S6Þ¹@Øée´»@>ª¢ÖY>?Àh‰@ÛèI¿©ÒçÃô*?êÇ5žd?õ'¡Æ
ëÑ¿àôÈý¿Î(•µßJ~¿æהܛvé¿Þ)–|XÁ¿ÞµñäíU¿ÔÖ[[	fAGNbcu3FGL J0447.1-25402MASS J04472149-2539302?ïüµÆ~‡£?0'"lVì?:QËEÂ?0'"lVì?ïìFº¤)?l©¬X?c¹E—÷öw?l©¬X?ïëŽÄÜñç?cŒeèµá!?dq;٘?cŒeèµá!?ïæARb?OGl4+°?i¾ô÷«/?OGl4+°?ïú¿Â"O?=J¹CgÖ?GÝrùn?=J¹CgÖ?﫦ñ_Âø?‹|Á»"wŠ?…C«~Ýü?‹|Á»"wŠ?ïí*0¼F©?hHõmzß?bÕÏ*ü'5?hHõmzß?ï+®ÿ?‰l÷
ãÏe?œšœ¬"?‰l÷
ãÏeAGN4FGL J0447.4-2747¿Üˆ¥	S)·ÀCbäѦÀ<SxM¸À="—jpÐ@ßÀ‹@ÓM"îê?Ø«¿Á¡u†?ïô%Á°Žÿ@Ð=0ã@
òi™ÌšM?î}I׺f™¿ítw Gô
?Û
Ú¤{Ë¿ëžñݨg=¿ïíØë¿[¿ï PØ_¨AGNbcuMRC 0445-278?ïÜl»GÇÈ?¡–©8îÀ?qÉ¢F·î?¡–©8îÀ?ïäAöš{—?€ ÂžCÏ?k¾	Œû?€ ÂžCÏ?í›uA?¡K¦ÅÇ·ô?³$c?¡K¦ÅÇ·ô?zZ?"cRIsÈl?¦ˆV‹‹?"cRIsÈl?ïï™+›Ë^?p^H©Gҟ?`fÔqó¤?p^H©Gҟ?ï¾Öìμ?"ì'¶s^?€JO³k?"ì'¶s^?ì"XNöˆ2?¨~ÉΝ?»]=ˆK¾o?¨~ÉΝ?붟@ný[?²&æ›k[?Á%'þD
"?²&æ›k[AGN4FGL J0448.6-1632?ÄÅu—© îÀA8:}ªOÊÀ9mÆÚD""À<OËn@/=ƒC@ò?ýq½¥è\?±]!™,â?­r¡L%@!
 ë2@aTåµ{ø?ïØRÂD³Ž¿Ê¥ªžú'¿à+ÄÿÎ׿¿Û6QØ7¿Új©Ø«þ¿à­#^ÔÌ¡AGNbll3FGL J0448.6-1632RBS 0589?ïþ¢'vge?ÕæËM^ù?%×ÜK$A?ÕæËM^ù?ïö 2þ[?Qž¾×èÉ?S¿œùJ$?Qž¾×èÉ?ïõÏê°ÚË?Zõ6ø‹~»?T`*‹™²?Zõ6ø‹~»?ïíRpæ)?Hˆx	~o?b­>ÿž¡?Hˆx	~o?ïüì7©Ã?-vlbJOÒ?8žA–:ô$?-vlbJOÒ?ïתæ•m1?­?"H{N?t*ŒœŒ7c?­?"H{N?ïòžüì
'?g·*°Œ?Z¦\}‰?g·*°Œ?ï̵ˆ7œy?e¿Ãúð?y¥;ÙâïU?e¿ÃúðAGN4FGL J0449.1+1121?ÞâÝN"ûÀ4¼«Oœ À8-e•†¢À;'·îvï@¶Ä¼2ã@ewS?¡âއ	t?ÁÇ­¾"¥¿@©qÁ
{ê@À×õŸÔǿјº¡|¿ámm "Êþ¿çga8)<¿ç¿]¾L+}¿ì§%pÔ)¿ðAGNfsrq3FGL J0449.0+1121PKS 0446+11?ïóISÂ?Uv"%u?XßÓ.«÷?Uv"%u?ïèÕºdÈà?qïLÞ
êŠ?g*E¸×Ì?qïLÞ
êŠ?à²?ËßjÝ?:¶ËG€?ËßjÝ?ïÕ÷"-HÛ?`ÂuOŸ?unöj€?`ÂuOŸ?ïÏNÖ?wá•uäXé?x}öK†q5?wá•uäXé?ï®ÜøF«¿?‰4æÀ˜?"HÁÝ~ús?‰4æÀ˜?ïe· VüU?'tA,?"Iñ°Ùh?'tA,?îÅr.+óŠ?Åú*5€?£¨Ý °cZ?Åú*5€AGN4FGL J0449.2+6329?—ýÈôú@'Ía€M˜9À9']Šõ'À;¬Ê‹¨?@ԂTƒí@íhžO?ªÐNâf<?·AªoT̋@Cf½Ë¨@C4ò% ÷¿Ú%a#""¿Ó**@Ejm¿á³hãh­¿ä¡÷ÁÃu¿åÎÀWs"\¿æž£Ä•ÇAGNfsrqS4 0444+63?ïüôVÐq?0D]Üåؼ?8_›U5X~?0D]Üåؼ?ïñR‹›²¬?`ð5"1­–?]Zè~c7?`ð5"1­–?ïàÄEGe?rJQþg‰?oé;€ÿ*Ø?rJQþg‰?ïÿ45Aå?<{Õι«?yXÁޅÃ?<{Õι«?ïû"n™]?9fù^Î?Aï¯ ôÍV?9fù^Î?ï°Ð'ä
?‹,0Ã=î'?ƒËû杲É?‹,0Ã=î'?ï¹:ïÈ­â?…+¡ž"¸Ü?±D	]	?…+¡ž"¸Ü?ïýÎ!‹•ö?'¥—í7|Q?1ŽóC§þù?'¥—í7|QAGN4FGL J0449.4-4350¿êœáçTýÀCõâŽÕñÀ6ä˒:*À:À>ð֗Q@vµú£IÇ?ûþÛ<Òf?'¯­|r?¯­DË@Ö"Ì«?@Lêt'š?ʜ­	ãل¿Ó¥"EO@¿ÜA¤ÕÍ¿×ÅP׈èq¿á*½]Äu¿ÚôZƒGsAGNbll3FGL J0449.4-4350PKS 0447-439?ïö9t÷›?^ìUl°ºÃ?SvEÙ2?^ìUl°ºÃ?ïð»"ô¡Ü?mJp…Pó?^ˆÕ¼™^?mJp…Pó?ïH†Z#?•§T«–&?–ï=Ùãb?•§T«–&?ï÷ÄÄYz‰?A§dgNÉ?PvweÈî?A§dgNÉ?ïøýÎø?Q¥7}yð?Mÿ6Âf]?Q¥7}yð?ïÐ|«æçð?†LScÖôV?wÁ©ô~Ä6?†LScÖôV?ïÂ$,&›í?ŠaíÑlSA?~íéù¡0?ŠaíÑlSA?ïè-£§9•?]³»´Aª¶?gÒ\2JÊè?]³»´Aª¶AGN4FGL J0449.6-8100?½ôç0–À?cà·õ¥À;À´%tÀ<ží$[)@ êÿ	àÔl@¦@×`¥?Ãþa"Õ<]¿½n¤ÁÁ?ù›ÞM'Ðÿ@*¸¡Çx?ïÿ¡ÁnT¿ïˆ_µr=4?Òed®¿ïõYÀÌä¿îO²
¤Ÿ?ïüV'TàAGNfsrqPKS 0454-81?ï÷Ò¶Š"í?qwÑh(?PZ'òî֑?qwÑh(?ïîžA&Än?dç¥1zÞ?aa¿Ê.?dç¥1zÞ?îåÕåOOž?–â"pÇÑ+?¡¢¡­ž»?–â"pÇÑ+?ïï:Á®î?Q¯ê?`Å>vÿÙô?Q¯ê?ïðôÍ8?g%6Jà¾?_òÖ®¿p?g%6Jà¾?ロܔì?BÁ¨üÂð?~ ²6*?BÁ¨üÂð?ïF¡]
?"XLL}¿Æ?—+ÔdÞ¶`?"XLL}¿Æ?ïg
á Ü?Šç*'8,?"\{Dޛ?Šç*'8,AGN4FGL J0449.6+3027¿ßîýy=ÀÀ"GýœÀ:4žÝ¦8äÀ;¸sQ0t<@	=-.@¬œ[ùŒ?Í/5wÜ?É9(Ö
b?þË|j´ª@å¨îÌ&	?ïßG"Ô@_¿å%èâ­â¿ë@óæ¿âW'X\¸h¿ïéÄ¿¸T¿æ$AÓ´óAGNbcuMG2 J044950+3026?ïÔn¹tÎ?ua›édŽô?uÈý<²µ?ua›édŽô?ïÕª
ÍZß?yS®—œX*?u*úºNЈ?yS®—œX*?ïqáH?ˆrEá™_?'ÃÝöüÝG?ˆrEá™_?ï'ê8Ìÿ?hýM_ ²?‹…qÌÿ€1?hýM_ ²?ï,*EMçê?œÀÀÈÀJ?šz·Wúв?œÀÀÈÀJ?î¥Eõ?¨AT:î'5?¡g£ë±?¨AT:î'5?ê餿¬?¶ÍŽÎñ\}?Ç ZmO?¶ÍŽÎñ\}?ìLiÌ3? äÒ*™VŠ?¿§uœ±žk? äÒ*™VŠAGN4FGL J0450.3-4419¿ÓüL»´:tÀCáþ!ÙnœÀ9z:э%îÀ;¶íª'æ!@\‡à‰˜@I©|e¬,?¶9Ô1;·?¸}BöÊ¢%?ûÕv¿yþ@æ}"¨¿×XÝ|Gy;¿äÓI¨Pí¿êŸ¾vÈ´9¿é–ß?–¿ìs§A¢â™¿îW…BI¦'AGNbcuPMN J0450-4418?ïý6¾qÙü?/ïp‰ú¾?6Jmã´Æ?/ïp‰ú¾?ï÷¹€Gk­?RÙÅ@¬ç?PŒÿ¦Åé?RÙÅ@¬ç?ïÊg>ŸðB?y>´†²õ?zÌ`­øã?y>´†²õ?ïý.ãþ?$f׈Åò'?7&ˆ²9C~?$f׈Åò'?ïùµz9›Ç?Mææ¢;ª?I*Ãýƒ–?Mææ¢;ª?ïვÌ/™?|Ra
G?n|j^kŽÐ?|Ra
G?ï{ñ«±ýœ?Žæðíñé?Ê†P°?Žæðíñé?ïï.
¡»ô?R‹Ëî0à?`Ñõ'JKò?R‹Ëî0àAGN4FGL J0450.4+7230?ì.qK-7@1x¢Ûa»À;µ'm,À<¦µ™ª@ê«5ÎC@Å+M‹¤?ÆölXmÕF?­‹RY?ãIþ†ƒ<`@¿̀ø?ï¢S².»Õ?ïä>ÙY£
¿ãÕµ¿'¿å&ÜÛ±¿í¬=Æþ?ԁHŸ¬RAGNbcu3FGL J0451.6+7231NVSS J045109+723014?ïûD]ÁÀï?@V+j1Q?Bî‰â¡³4?@V+j1Q?ïðë|)5?`TP‰
M\?^)ÖÑ?`TP‰
M\?ךּ¿óº;?~Š‰©µ;?"ÑP?}?~Š‰©µ;?ïèòJ"Tº?P'Äãû_?g
µwªR?P'Äãû_?ïó2{—ò?VÓXÊIúE?Y›cäœp?VÓXÊIúE?︔M@?…"êÐ=я?Úþ7VÅ?…"êÐ=я?ïœ-dÖÞ?‹2o"kŽ?ˆýô±o?‹2o"kŽ?ïªÆpÎZ}?wŽ'«ÆôB?…NcÂŒá?wŽ'«ÆôBAGN4FGL J0450.7-4938?Ô2z)'tÀCÉúëÄÙÀ;Pûð¦Æ©À<ßþŽæ¸0@¬áUoô@>µÛ¿ê?ųZµÙ[¿–©@€£©h?ÐëÙ!ÄËÌ@Y¶o"5Ò?ï|š…Qãø¿ç8~–ÞÔ6¿àžvþdŽ¿äZ^»w9ó¿éÀ:SÜ?¢{•w öAGNbcuAT20G J045102-493626?ïø'3?ER CT5è?M¿»èÅ«Ÿ?ER CT5è?ïöBÚ¶?V3å÷÷a?SzüÉlL?V3å÷÷a?ï֔Ò	¢–?tgÓÉÓ`?tµ–ï€	?tgÓÉÓ`?ïù÷Î`Ô4?/±Þ(+'?H Ç#Ïc?/±Þ(+'?ïÚPŸïbé?pé¥ÐP'E?r×°­#¡?pé¥ÐP'E?ïݧ'¢ü¼?p3ZŸÖ?q,6¯1ï?p3ZŸÖ?ï¸z¡Bµ?ƒçF#ƒ?áW½ø–?ƒçF#ƒ?ïäN¸ía?XŒaR£a?k±Fÿ®Ïs?XŒaR£aAGN4FGL J0451.8-4651?ÄÎå>;W£ÀCÀe¾ ºÀ9ßõ}ÅþÀ<A©n*@ü3öQ«n@ÿ#¶?¼¸ì"x?¹ªiJœ[k?ú|±|nX@¥CžNl¿æ‡¸Æ…Šï¿ã!'fw-^¿ç(èÁõÙ6¿ÝÉ%8HÇ¿ïþ˜÷³*d¿ïù|´†…AGNfsrqPKS 0450-469?ïý¡‡é\¿?$‹A1 3?2óÀ"ìá?$‹A1 3?ï÷ª‹Ú>O?Q¦¢ö€Õ?PªèÒ4c?Q¦¢ö€Õ?ïã-î$?o?H?^å"?lÒ2¼Ó¡?o?H?^å"?ïÿ"|üÕÔ?°­Gñ?à·ªLöQ?°­Gñ?ïþb'W—'?!Ž´ŸGuî?)ÖÝ¢™t)?!Ž´ŸGuî?ïߞíÛ) ?qªå+?p0‰ )à?qªå+?ïáeüç¥?z7%
‡c?nñ™Ýü'ë?z7%
‡c?ïþãåb? ƒlÔc?!Á«U)Ý? ƒlÔcAGN4FGL J0451.8+5721?î$Y §¢=@ £úLaØbÀ:ã9º5ñTÀ<{‡(}Î@!³§ú/†€?øR7y…?Ó4ÖÁ˜;K?ØCP·¨xZ@óݗö+k@¡vÈ3_ÿ¿ÐO¯j¼6}¿ïÿèþ†®/?ïý›6QË¥¿Ôný?¿Ò÷si"(¿ë°Ú=x±mAGNbcu3FGL J0451.7+5722NVSS J045148+572139?ïû››žÏ?;->"l?CŒuÃá?;->"l?ïãívv»?rå"«s?l‰Éݤ?rå"«s?ïÊêì¿Ó·?vaZ¨¸‰?zŠ‰¬t¼7?vaZ¨¸‰?ïÓéO%q?bùyéÿ?vrÝ짂?bùyéÿ?ïúŒ«/?Af"0¨2?EÍSŠp?Af"0¨2?ïIєK•Ä?¡¤¥`S%7?–ÅÍ}lj?¡¤¥`S%7?ïÍß¿B˂?€t•ðNy?y i˜ÿ"?€t•ðNy?ï"C!E}–?!>°"-Ü?‹/7¤QƁ?!>°"-ÜAGN4FGL J0452.0+2100¿ê<Z']À,ø§ayWÀ;YzŒŽ\À<…ñÓ'é@"³Öe|Üu?ùQÉ÷/væ?Ï+=…òrÏ?¿!%¿'6|?òkÓyq@sœ§Àù°¿îÂÉ.4¿î²;QæM?ïÿXÛch…?ÝÇ×DŸí¿ã¥u«?q7k¸FFAGNbcu1RXS J045214.8+210307?ïÿ(vŽ3?
ú áÚ¢?ñ1Sߤ	?
ú áÚ¢?ïôæ<Ɩ
?XÛgYª?V3†T—UÍ?XÛgYª?ïó+™"nÀ?bïw%AÚ?Y¨Í]Ó/;?bïw%AÚ?ïõoîôJ?Goõ|:`E?U #àԜr?Goõ|:`E?ïþøm†ã?]Ç÷́ü? y&dƒÌà?]Ç÷́ü?ïÙ&
Ÿ"Ÿ?{¼Óùóf·?slùNr@E?{¼Óùóf·?ïø!Ï*¡?Vïî¼íûÖ?OxÂSèü?Vïî¼íûÖ?ïä"·ÃƒÖ?f'šè¥?kÝH*ž1¬?f'šè¥AGN4FGL J0453.1-2806¿î-¼§CXùÀB"Â	$lÀ8'Îï¼»ÞÀ<©@։å@A|wð@P­Í-DÝ?£¡?Ö.ËE?¸ªÀ³cð@¼Ý!®¦q@ùÃOöb¿ÖE»ámÛ¿äêB‹@¿èô¾þØㆿê"úÞ­õÇ¿ëù÷2ú(¿ïÿÓÀíAGNfsrq3FGL J0453.2-2808PKS 0451-28?ïûæÆ0=?:31žCf?@dècV?:31žCf?ï÷\Ε­Y?QpQóy÷?QFbÜä]?QpQóy÷?ï¼f[1\¢?~µ­3ò?€æi.Ùc‰?~µ­3ò?ïþK5CÚ?]çúaf?+O½ªØ—è?]çúaf?ïþ?òÜ?'Q`qça?/<á%·?'Q`qça?ïÚ³/Aáø?€Q¡ÏpZ¤?r¦h>ÄX?€Q¡ÏpZ¤?ïÓg\@ÙË?€óñ,¿,ü?vLQ¿ö²?€óñ,¿,ü?ïúvh3'v?=WLE:‹.?F&_Y×þ?=WLE:‹.AGN4FGL J0453.1+6322¿Õڂö9á@(V|ᛑÀ:S±E‡ÊÀ<+¯BxJ"@ ¦ˆgB.@zlãX)?ÁJº"üq?›-¹ÌƒÁ?Ýú$Á‡@émÇXÅ?í£J¨š¾¿çðÇþ±Ì@¿èú)(î6¿ÑËaè¨K¿ä!æ­j1¿à@"°%ÍAGNbll3FGL J0453.2+6321NVSS J045312+632117?ïþƒ)&?Ï%ÙÁw@?.NÌU¢?Ï%ÙÁw@?ïñx<F?cËq&Œd?]ô"ô¾?cËq&Œd?ïû_Ýqq?1¬ÂhU"-?Cþ€ÍØòV?1¬ÂhU"-?ïóór(•?>"®+Ä]?X$í?>"®+Ä]?ïþy'ç®-? øs‡ÞV*?(m''kÐ? øs‡ÞV*?ﬖ`ÿõ?Ž¡ÜËa?"ÚgÍÁ)Ü?Ž¡ÜËa?ïüMGJ[2?Iò.2=9j?=•Æ´
é?Iò.2=9j?ïÕg ܪ¢?a—!ûk†b?uLo›ùƒ*?a—!ûk†bAGN4FGL J0455.7-4617?é"o'*"zÀCi˜áõ²À9
¥ÿ©þÀ;ðšrÝm.@&¢†}20@ÝÓ4ÅÚj?§!­¤¾e×?´âÎì·£Æ@	ÿG¶@yX«gÍ¿¿ì 	·¿ä±Ö;áWž¿ç¥c¯˜	¿çWìPÓ¿èŒYÙ¿çƒO
)N®AGNfsrq3FGL J0455.7-4617PKS 0454-46?ïþÚ+?%jóê½xâ?.'Yð£?%jóê½xâ?ïø<ÕÉK?R7=r'?Oëç†çÿ?R7=r'?ïáý‰ê5O?rÚjßçŘ?nuÜA©?rÚjßçŘ?ïþt3ÐßM?'@جœÛ?(¼Â¢àõ•?'@جœÛ?ïýÔȧÏ?)GÑj;?1_úðÑxù?)GÑj;?ïÝÜXñx?s$w–ãO?qõC	$L?s$w–ãO?ïÄUvmßE?~ZÍm?}ÕD²bñm?~ZÍm?ïúî'h?<ÃZäo|m?GˆH=¢ü?<ÃZäo|mAGN4FGL J0456.2+2702?ë0´Ö`õ8À$0H@áÀ9µ~q'
À; Œ‰ޚ@•tÁrüw@ïÇ£˜ ?¼xtŸ¨ì?Æ.ëzâÊ:@£É%x_@ phó´m?çÜ"N‰{¿Ü^d¤ÅFÇ¿ãc3vO¶¿æu
þÆD¿èå@6&¿ïÿ¯b® èAGNbcu3FGL J0456.3+2702MG2 J045613+2702?ïèÑÃ+¹A?žÜ®…þ ô?g.<—Ížÿ?žÜ®…þ ô?ïñˆí¾£®?a!E#rè?\î$´™?a!E#rè?ïÉ?GP?wòõÚÒéÛ?{`\n8jq?wòõÚÒéÛ?ïîq./W?Cx7‰·á¤?aŽÑÛ§ ‹?Cx7‰·á¤?ïäˆ5:´?d—'¾{Ìb?kwÊÑÇËÃ?d—'¾{Ìb?ï¹Äöz×H?ŽúÃ:ÁŒ?ŽÂd¹Ê?ŽúÃ:ÁŒ?î"dÈp`?šÑ>í?¦É³|i"?šÑ>í?藍	HÂÖ?q'  Ñs´?†×=¸a?q'  Ñs´AGN4FGL J0456.3-1634¿ä"bÐäÀ@^JÀ:Ý'nâlÀ<›×5Ü@ÎFtƒ‹?ü½úºpª?Ð
]O¼V?Òrsºâ¿}@‹G&/>²@ÃU¶ÀÆÚ?チ_æðe¿Þ51e'Ìù¿Û§Î›Ya¿Ó)<ÅS¿èÙÊÁÚ«]¿áœ]=ó«‰AGNbcuNVSS J045618-163552?ïöù{×fÚ?K%H•?R
Šë¼^?K%H•?ïñQ_R­?Z (æê_y?]]A8TfQ?Z (æê_y?ïÃÅÎŏ0?v'…²‰c?~—	8?v'…²‰c?ïд©Ñ†?ZGìVîŒÛ?~7¥¨WŒÙ?ZGìVîŒÛ?ïæºfîk?gïØkµe?iE™©ì–?gïØkµe?ïÆfî:tŠ?7	óDþ?|̉!Òä?7	óDþ?¶¼©?šƒS§´ôÆ?¥—"œ€€x?šƒS§´ôÆ?ï7þŸã?ƒ$Š‰Àbx?ž,Õ?ƒ$Š‰ÀbxAGN4FGL J0456.4-4043?ï•4•¼rëÀC:-ƒÆÉ~À;oºzº±AÀ<ËÆ+ÈÛ§@úu.«9)@ü!ƒÞFr?ÅEÅÇtô¿±Tÿ5Õ¥?élґ1ì@ý½Èäá¿å3!€nÅ¿ìé ¹³ë¿ÞžOv_Ø®¿ÚMõÏ¥¿êkŒÞl²?ËÞ3<ˆ]AGNbcuPMN J0456-4041?ïý'¢1BÃ?6ûižÙÑ?3êïJ'µ?6ûižÙÑ?ï÷è÷б‰?SÏ×µ³QŽ?P.2¡î ?SÏ×µ³QŽ?ïڃé¦n·?x«}e2%?r¾
Ü(ä?x«}e2%?ïÿ;v˜ó?,ÞҖ?';³÷?,ÞҖ?ïüF‰ÉM??¹-ón•¯?=˱ØDÝ??¹-ón•¯?ïÞ1לL?|ëÊB:?pçIT²?|ëÊB:?ïÙýf¿ôï?9#9¤g?sLŒÇ¸_?9#9¤g?ïúë-µð½?:±ë'ñî?DSHq¸2\?:±ë'ñîAGN4FGL J0456.6-3136?á 5!ŸâßÀB‹;BÌ-kÀ9×Þuk¼çÀ<}'Õ1@êÅÝð@¥qŽ¸•?´8=´›É?µ8æÒÝ]?ùô3xÓPu@Q/¹¬²?×Îÿ¬óéq¿á­w!t™Û¿çøÃ*Œ›"¿æm¾ÌeŸ¿ê½ÁÆßM¿ïÿ°_ïÉAGNfsrq3FGL J0456.3-3131PMN J0456-3135?ïü*éÉg?2ÀS¸Ý¶?>¨¸Ã¬n?2ÀS¸Ý¶?ïõˆz.ç–?SøA#¨"?Tï
d¢ƒ?SøA#¨"?ïêã0=h?Yitp'ÎÏ?eô‰È:?Yitp'ÎÏ?ïé˜<¢G¾?S¤§íTä¬?fgÚ1a§?S¤§íTä¬?ïùŒ
1S¬?Fˆ´!`Ê?IÏ×ë¶ÆÜ?Fˆ´!`Ê?ïÙ« ŠØ?u¢1Y"?s*/ØІ)?u¢1Y"?ïÛhˆ›?züÉ܃×A?rK¼Ýzy?züÉ܃×A?D&©?w•_]h§è?‡ûX®öU»?w•_]h§èAGN4FGL J0457.0+0646¿àq0wt´;À5«Þ灃ùÀ:­¸4TÀ<ùÅS[È@/©RtA@¯U!š"?Á­‹¾åƒ}?ºF6mÐ=?ô—'ML¹í@ç~­Úï$?åïB]r¡Þ¿ÜK"]xB¿æ韀äA¿éå.X•¿éO€pÓ¨¿ïþcèݤ‹AGNfsrq3FGL J0457.0+06434C +06.21?ïýR	HdY?Tƒ´×?óÝ?5o¶âo	'?Tƒ´×?óÝ?ïöQ.àú?U€®µŽXz?S]¡Æ	ÌI?U€®µŽXz?ïàzã[J?i[êðÏå?o…ÌIÞ0?i[êðÏå?ïýHÑ2À¥?!…+Ñk½?5¹v)Ð¥?!…+Ñk½?ïüz3'?5ÝhP×s?</7NNV?5ÝhP×s?ïÝD|PH?sabü
©ú?q]ÁÍ¥oÓ?sabü
©ú?ﯔj…¯Ø?'ñK2¦ ?"ådj?'ñK2¦ ?ï÷ñsuB¢?>èUBþò?Pz»ˆ?>èUBþòAGN4FGL J0457.0-2324¿éVXÔNîÀAs;÷'À6q%»{k±À:øu/@­!­ú¤¡@ξú|2?€a—Ó#‡?³YéA¢@*x®I#`@ ȋ÷o¬¿Æ律4ë¿ß3âÂ\†¿ä~!nÑ¿ã¥cœ‡Š£¿ç{4ßZÃñ¿é@|ÇÑ»IAGNFSRQ3FGL J0457.0-2324PKS 0454-234?ïõ!¨"–?Q¸šP!Ð:?U½ø'~D?Q¸šP!Ð:?ï± ÈË?—8Ž©àëf?ƒ—ߐŒë6?—8Ž©àëf?ï|›ûþ?"~Ï'•Ò,?n"<?"~Ï'•Ò,?ïíK&2Þh?i1»)-k?b´Ù¯ž?i1»)-k?ïôHâ>p?R¡{'xí?Výn›¸.?R¡{'xí?îß3ß«v¼?´¤M\_¼?¢ÂýI?´¤M\_¼?ïÉ´&9Œ?"ÙµŠà?{%¸Aõ?"ÙµŠà?ïB`¹ÂóŸ?"sÞs­?—³èÉYZ!?"sÞs­AGN4FGL J0458.0+1152?ïWF"Ó¥ôÀ2¦šíV°À:îê'ò#À<R1Xg @!ǎàV?ýÛRUÆÜ?̈́`¢W-c?™8 °d?¾žœ7ً!@-TÔî"X¿È¬Ãœã%¿ëÁ!h/"B¿ëÍÌsáy?Òó½‰bë¿á‡¦RÁ¿ÎÿùŸé"ÚAGNbcuNVSS J045804+115142?ïþÇb•v?¸sxÝ/?#­øc†2?¸sxÝ/?ïö¢]¯Õè?Rí¿hçœE?R»DýɎ'?Rí¿hçœE?ïïåQd1ê?X††¹K?`®­¬
ù?X††¹K?ïû	¶©û?/§£"Ï·?CÙ'ëK÷?/§£"Ï·?ïþS"%Wí?$Äõ¾f9?*ǽN%H¿?$Äõ¾f9?ïÙ¯M#ãú?söyUì?s(Y^?ÏA?söyUì?ïôÚ?gΘWcäã?a|A3ñÝõ?gΘWcäã?ïåÄädÞ?a:†‹åCï?j÷:úžâo?a:†‹åCïAGN4FGL J0459.4+1921?ïÔ5ŸcÍÀ, æ)•$ÀÀ;"ù÷¨À<BŠgÍn³@!ë‹Ô´ù@!Mø±W&?ÎM/Ége?‰régÉN#?À&¯X‡@l5%Ñ¡¿µ@cÖ>;?Û7½;_QŸ¿î˜Ù`ð?ßgk^Å"¿Õ;ˈ).Í¿å@¿ã°>AGNbcu1RXS J045931.5+192242?ïþ'¿à«&?!9Œa½Å™?&Óþè¦c¬?!9Œa½Å™?ïögœ¶x?UÒŸMÆ?S0ÆQ̑?UÒŸMÆ?ïí^{$S?^×À$ٍT?b¡"Ò¾¥?^×À$ٍT?ïþ˜¬‰¶M?©¿Ö Ï?&u8s
G?©¿Ö Ï?ïýêíQÛ?/ú¶>U=Ÿ?0¨–®é_‹?/ú¶>U=Ÿ?ïÚÙs?u¤å»?r"Fu-Ÿ8?u¤å»?ïé§'îþÈ?qQ™fDÀ?fXØa¿?qQ™fDÀ?ïùp— MÆ?CŽN4?J=¢Wð5>?CŽN4AGN4FGL J0500.1+5447¿ïùúÙ̀@'r%·I®À:žÆ3¡îÀ<,©ã"¸¯@Ƃe n@±Âþñ´?Înø†9?À±½½:]Ÿ?í=Àgc¼@Y9Ô1<¿ïÊô Pm?ïºiúÊ¿èín˜dt?²òpËD7¿ïÿø]ˆò?ïþ÷ýÖÛAGNbcuGB6 J0459+5441?ïßa»ÃK?…ž!`g§?pOp"ZV?…ž!`g§?ïèÜâªÁ?lÝIZ²?gí#•??lÝIZ²?ïZÎÎbVÀ?Œsê×{†Ç?"¦&7$Ãÿ?Œsê×{†Ç?ïá–iI«×?\:#4‰?ni–œ7!`?\:#4‰?ï²*V±?†òGa'¶
?ƒuj†¢Ä*?†òGa'¶
?ï0¯)›&Y? çlz>Å?™êÓzl×? çlz>Å?ï'SŠt?•p*Ímu?œ_O·Fv?•p*Ímu?ï(ºuv›?"D¯ƒüÿd?šè±H¦¦·?"D¯ƒüÿdAGN4FGL J0500.2+5237?¿–a°
Q@fL¡™B\À9ÖI°M:EÀ<ïH!×Á@!\$˜Ö¸?þŒý"$½?³ÇÝ_þ(¡¿'¸îª_å?߅&šôb"@-Ÿ¿ÛÓCÁð?ïò¥­Û¿è]¶Šk¿Ý– 7˜s¿×^ÎA–ù+¿ËŸ¥aÎÒAGNbcu3FGL J0500.3+5237GB6 J0500+5238?ïúÅ]í›ú?=CƒïâN
?DꇘŠž@?=CƒïâN
?ïèiï:"'?oÞ¸ð‰Ã?g–ÌKµ›?oÞ¸ð‰Ã?ïãp»‡ˆ©?pšuQ…™?lDxwWr?pšuQ…™?ïÞÆ.?[º´e©J?pòø;0Ñ?[º´e©J?ïôe+¨ê?LµÀ]å˜?W5Ãl5C?LµÀ]å˜?ïqáöøW?šâ0ö@?'ÃÁ>õ&?šâ0ö@?ïÇH7–.?þï"þØÇ?|[äÿ¨û?þï"þØÇ?ïxœÊâ£	?¬…Æ7?ìfœÌfç?¬…Æ7AGN4FGL J0500.6-4911¿ÖÑøì̃ÀBý@=ݱ!À:­Ž!–R½À<Ÿù¬ÿ§ë@ [»=XP#?ürùà0W?À5AU_ØÙ?¨äEdc+ô?ì¨OÌû@Ø×¾˜V£¿ïEFáeá?ïÒÖ0ù¿àFÀ¾Ìƒý¿Õ0ÀRŽ¿Ý"¡}=ÃZ¿ã•[$AGNbllPMN J0500-4912?ïÿ''·æó>ÿ£pã¦K?_BNî'>ÿ£pã¦K?ï÷I‹lã·?UüÃpÊ¥?Qlé]2Rf?UüÃpÊ¥?ïø `P?<Z"T2v?O‰€$'+?<Z"T2v?ïý¶:Jdä?Ü}-Æ6§?2N+çÙ-6?Ü}-Æ6§?ïÿ9_J?QUÙãx?Þõ>J*î?QUÙãx?ïÛ AéÚO?;º?roß3 ©?;º?ïùǽLí?Td_B^3?HáZjU?Td_B^3?ïúU3ìŸ.?9ùchîa?F«0†¯ü
?9ùchîaAGN4FGL J0501.0+2424¿ãâÏ—àÌÀ%Š|àü.ºÀ:à{ö£ðÀ<_c>"¹†@!W¯K‡'Ü?üÄ<"¸?̒üÇf[?Îìì¥@°ý¤?÷éä4È^©¿ïÿôA…ÜM¿ïï&"è±?ïÿü9¡â=¿Égâ<u§¿âð!愯¿Öv"œ;AGNbcu1RXS J050107.1+242318?ïüžÅþQ?5ˆRû©y«??ãxvËS?5ˆRû©y«?ï¾ý?Ë
ð?…áJÿhè?€@°4"?…áJÿhè?ï½ßã;4p?Û^vµ?€ˆ.>?Û^vµ?ï*{öèÌ?"#ÆÏIä,?š°+}v?"#ÆÏIä,?ïú›+
4?Fº«q?E"¾Î?ûÂ?Fº«q?îéËÉu2?±Iä~?£ÅcDD"Þ?±Iä~?ï"Ú;º7?ŠÓ_À`×?ŠÉq=b*?ŠÓ_À`×?ëÕÐÇXC¹?²@ó}¸'ÿ?À¨¼âžñ?²@ó}¸'ÿAGN4FGL J0501.2-0158?íÂ"kÀ9J]ž@ÈGÀ7­†!ÐýÀ;íZQ@x…v!@$Q2øzÑ?–Ö+Ú¤Q?¶"À%@ϼ¡Ÿ@‹F¿Å¿Êɹà<¿âl•õ *­¿å©Æؗk¿åFC¡+¿êңܺî¿ïÿ½ÅGóAGNfsrq3FGL J0501.2-0157S3 0458-02?ïò"ºÂç¤?Y+ˆ…§J?ZöŠVtÇ£?Y+ˆ…§J?ïí¦…6
?ršyÓݹ?bYÿ»bS?ršyÓݹ?ﺨe—è?$eñ'i?~¢«í€_Û?$eñ'i?ïýf|O –?)Æ4&KZ?4Ì·bÅÒ?)Æ4&KZ?ïîÙtJD?]ŸÒÓ×ð?a&êL|ìÎ?]ŸÒÓ×ð?ï¾ßd\©'?hôêq?€H&Üž?hôêq?ïҌ•?»Ň7?v¹òTe?»Ň7?ïõt÷S‰?Mgö'÷?Uژ	?Mgö'÷AGN4FGL J0501.7+3048¿îŽóðÜÀ@eށ*7À:hÚà‹ÆrÀ<¼²£UÛ@!aB|§E@	ý¯Ã¨?¾!°¿Pˆ¿¤¬Ž¾Ê*±?äõé@ Ú?ý÷þyX1?¸Öf~'%?ïËKøüր¿çKlD̸«¿ái%}½ðç¿ÛÀ-Ëë%¿ÌæFÆbûMAGNbcu3FGL J0501.8+3046GB6 J0501+3048?ïúڄEt~?6m‹ۂ?D•î6Ç?6m‹ۂ?ïæâϺà3?n6K@Mõ?i0? m`?n6K@Mõ?ïìXÙ¾€a?dzÊhÇÔ:?c§&3Á.¦?dzÊhÇÔ:?ïÃÊùŸ$?d-¡÷ª§¤?~ƒp~v?d-¡÷ª§¤?ïôAÊµ?O 
¼Rå?W|k§î?O 
¼Rå?ïiÀy

£?¢LF,5ó?'ÇðÛO•?¢LF,5ó?ïâ<(á[á?s"<FNZ?mÃ×X]Žw?s"<FNZ?î‰5R)n?–à¼P¥JW?§lªÞq''?–à¼P¥JWAGN4FGL J0502.4+0609?æóöªÊLÀ4Ü
Ð=š•À9ÌTæ³^À;¼Ñy÷Ü@:꘺¡|@jŸ±
Ï?¿Ô‡×$i—?•[ÂéZ]?ÒØöî‡@çzÊÒ!¿Ø¿o˜¿ä˜±<MŽ(¿é"ø!å-¿åG†§NŽ¿î"6©	y&?Þh!Q‰`AGNfsrq3FGL J0502.5+0612PKS 0459+060?ïü _ºx?=sŞÅjÙ?:ýÑ-¸'?=sŞÅjÙ?ï÷7"s?Tm;0yc?Q×Ý3cºÿ?Tm;0yc?ï܊T­+r?iY=ó)?qºÕígB?iY=ó)?ïþÀ՝«Í?——,ø³?#ò¦Fð¯?——,ø³?ïø,­Ä/+?R½z³öE?OMIžÚï?R½z³öE?ïß@dÊ?}|—³kùâ?p_͘î.·?}|—³kùâ?ï¨Egyr?…Þ!tI?…î¦/aéë?…Þ!tI?ïú{ilj?>É,Àc™?Gþ:¢?>É,Àc™AGN4FGL J0502.5+1340?Ü^qš¢IÀ0»)^ž	À:&=²èöÀ<0B½ê²@)û'êV@rÜ£Úe<?Á͒švä8?­Ê­¸µh­?뢱Èd@¶5?|푿²çgWÒú¹¿åœ|m8è¿ÝïU"qD¿ã%‡
¥Úð¿â<
½s=¿él¯áY¡²AGNbllPKS 0459+135?ïýÀEæû2?'uA©xHä?1ýÐt–S"?'uA©xHä?ï÷PQbY?SJ{'7a?Qé_ƒ¶ìÛ?SJ{'7a?ïõCî[,?bhÔP|?UÙxA†8c?bhÔP|?ïú£—Ó?*Þ@Ó/î?Eq£(
–?*Þ@Ó/î?ïüj´©ÀX?6T½Î×u?<ª[@ìüç?6T½Î×u?ïÖ 4Ë07?€ŸšlFÁ?tï厹8•?€ŸšlFÁ?ïöÆÌ5UÖ?c@3	ŒW§?Rrgy×t€?c@3	ŒW§?ïì¢ÚØJ§?P¹"²>t?c]%LÑ!?P¹"²>tAGN4FGL J0502.5+3438?ì<䗙º&Àe©>ê!À8ïíO#SÂÀ;m·‹(U@¼"ŽðsE@‡z³$…?±1é\$™?À9×|©ñ@_;©#z@(ÿZ¾'w¿ÃžvãŒ+ó¿Þgö^k›/¿ãºÔ¢Y0É¿äÅÃù¿t¿é"´À;™ß¿ïù\wÐ6AGNbcu3FGL J0502.7+3438MG2 J050234+3436?ïù¸b?C+…B"?K·ÈâµJ%?C+…B"?ïéõMZ·î?tÝځb`ˆ?f
²¸…â<?tÝځb`ˆ?ïÉvA¶êÉ?v%êʌ?{DßBÇ+?v%êʌ?ïçHR÷k(?Mߐ®Àž?h·¬ë¸Ä?Mߐ®Àž?ïÐ#îò'?tæìIq
‹?wöíþçÏL?tæìIq
‹?ï^³v˜?£k`$œ±@?"?i'äËQ?£k`$œ±@?ííÙâ´ë…?¥"o)@?°'0ì~eX?¥"o)@?ï}MÌçz?wüÔo¸"?_6D«BÉ?wüÔo¸"AGN4FGL J0502.9+6533?çG=:j@,¢ÿm3	BÀ;B§½HËKÀ<¿]K4²@"<}ðÿ1?ú4ÉÖxG9?Îý"û|ã€?µG@†Wó\?íà8Ÿƒ¾f?ã£éõZ=A¿ïê¤N(ÿ¿ì-ã}"S¯?ïý©®º"¿à>qTÖò¿Ô;‰"%¿©æ"'ØäAGNbll3FGL J0503.5+65381E 0458.1+6530?ïþ}¥áë1?"§"øÇ)I?(%¢=¨Ø™?"§"øÇ)I?ïŽÑâ`\â?"ÝbÍþƲ?ŒK‡kXcz?"ÝbÍþƲ?ïÅv¼ƒ)?ƒà3
øÖá?}D¿@KÍ?ƒà3
øÖá?ïçŠ=[*?Š(ï®}?œ£¸Tš·?Š(ï®}?ïþ5%.kV?2ÿÿqE?,­¯è_C±?2ÿÿqE?í¼6dk—?¼m$	Žbô?²LÝñeÈ?¼m$	Žbô?ïà·Dœ´y?wËø©ƒùH?oH»$·È?wËø©ƒùH?ëÿW"ž	?±Ýwö|?À£u‡ãÜ?±Ýwö|AGN4FGL J0503.1-6045?ïø¼âÃÀBG¼Â"çÀ:Ó^†žSÀ<4¾ÓåÅÂ@^Æ1Ó@.v]Tní?ÓÁ1ùwOÃ?ÙE~ð ç@`Ũ]_@†lQ÷?ïûŸíp±¿éq'Šˆ"ž¿èîwÂYV^¿è(¶½–Îä¿æsûŸóû»¿ïÿ.ÿqå¡AGNfsrqPKS 0503-608?ﴘV´¨Ð?¨=gyíÉö?'ÙêR}Ö?¨=gyíÉö?ïÓ»úþŸ"?ƒ†(ÝF¨?v"o'*"?ƒ†(ÝF¨?îÇ,ÃbH?šR8Ԓ&?£8¥Âw?šR8Ԓ&?ï¬xL›Ú?k\I<*Í?"áí×y\?k\I<*Í?ïèÓ9^¬š?s¢óðˆ*?g,ÆãKåÂ?s¢óðˆ*?ïïڐQ>?¥4ã(F"?œÂª†<J?¥4ã(F"?î*Ñϸ[ô?¡ÛDøY?­RãžYÃ?¡ÛDøY?ë77ß6Ô?°)"¤Tm?Ã# ƒ$¯"?°)"¤TmAGN4FGL J0503.5-1116¿ë½Ô6xÀ=âÅ\–À:˜Ä0FéÀ<id»k{y@ žMQü?ýHò'hûl?Ď:?ìÕ?¬
rIÉw®?æSò@#Ü~@'Ä{D™ã¿Ý'NÜÜåI¿ÜK(\ëhn¿ßÁí@	ÛK¿Ñ·üƏ›ê¿â=U–4ŠK¿Ôf%ƒ-ùAGNbll1RXS J050335.6-111504?ïþY¡ï»?(d³ž?*oä!t?(d³ž?ï÷Fè
¯ ?Q½õu¸ÀÞ?Qr/a0`_?Q½õu¸ÀÞ?ïø\¥í•?<N‡0.hæ?Njþ*¹?<N‡0.hæ?ïúðfÚÕ?.OžUv•?Gœ>'Ñ?.OžUv•?ïýõ'^Ь?" EXeœ0?0Sì|§3?" EXeœ0?ïØF	y¦?€Ì2h?sùÜÝœú?€Ì2h?ïû¡Óh·?Lk$q¤¹?Ax±Ó&šJ?Lk$q¤¹?ïëlJ+c?T)éiÚÉï?d"µ—
¤ó?T)éiÚÉïAGN4FGL J0503.6+4518?g"Nô2V@ŸÁßeVÀ9¯Üöæ{ÊÀ;Üè,¤£¹@ ¹uj:[q?þ•i‰0–?¿â=ž4?»ïÒ Ì=Ü?ý2Ú}wØ@%™¼Úç¿ì¾²Ã6K?ÛS®=j™§¿ßväOö7¿Ú"¨~cÞ!¿âX>à»l'¿âì&ďçAGNbcu3FGL J0503.4+4522GB6 J0503+4517?ïü‰‰½>Ë?2a'æª?;³²‰?2a'æª?ïՙÖð?…äyÇÿú?u3m2ýë?…äyÇÿú?ïïyÆ8Ô?c0ñQHíd?`†9ËiԒ?c0ñQHíd?ïÁz'8e2?bÊ檃ˡ?B¾ê¬ž¾?bÊ檃ˡ?ïöX?˜W‹?Kã äm?SO€ÄR)>?Kã äm?îyª³ÈCü?²"l¬h¸­?¨eTÄW§??²"l¬h¸­?ﰘë+š?‰‡NÝ@‰ô?ƒÙÅICíu?‰‡NÝ@‰ô?îáN6øBO?ŒqÃØcW?¡ë{Û?ŒqÃØcWAGN4FGL J0505.3+0459?è˜óò´­À4Ü9ÿÖ•À7jD†AÎÀ;öÍ0 @ØF·õOM@'Ï] Å?•€RY#?»\•­%è@#VŽÅ*A@ÕhÀÞ­¿Ë*(][Œ¿àèû6l£—¿äüÒï%½)¿åÂψh﮿ëQþ'A·¿ïÿ±[W>«AGNfsrq3FGL J0505.3+0459PKS 0502+049?ï×w€óŽ
?sÃ<…Æ?tD?o‹Žù?sÃ<…Æ?ïä+Ð,A–?x,	\®¦?kÔ/ÿ¹i‡?x,	\®¦?î'è&3_B? šA¨št?¦Ñ}›î$å? šA¨št?ïú-V‹Ž$?Cªø¥²"ž?GJ¥¯±µ;?Cªø¥²"ž?ï¾z'1&?|bò4µÍ?€aX•Ü`j?|bò4µÍ?ï«N¤l +?—º@JvZu?…,Vډ!G?—º@JvZu?î†
¥eÖ? *ÂGùï?§Ÿ/‡ap¤? *ÂGùï?ï×[)Ë?o!\‹7&k?tzRnœFÆ?o!\‹7&kAGN4FGL J0505.6+0415?Åðu™½´À50ɧ~^«À9Ì1p»SÿÀ<KŒÆL€@ ËE05ÒË?þÇë¼|?¼¦ÂÞ¼Š?¬.Eã?ï왡&UÕ@.	™Üµx?ïÒá锄¿áݳÍêÚ¿ä…™1"οÚ{$
¦\¿Ú;¼ïŠ¿âsÂóáAGNbll3FGL J0505.5+0416MG1 J050533+0415?ïûת~÷µ?6wcL˜dª?@¡WEÑ?6wcL˜dª?ïôÖ1-'3?U0V¨ç?VS¥±™¯?U0V¨ç?ï蜄±ë?g£i°èR?gc{Þq\³?g£i°èR?ïܪw¯±U?Wƒ‡ã|z?qªÄHs©?Wƒ‡ã|z?ïöï¢cå?E?/Ù»yØ?R!ü`'†‹?E?/Ù»yØ?ïÚ=ˆÌ—É?uðh)×aH?rá;ƒ¶›Ä?uðh)×aH?ïØ+ö(ê?z"wÞ7Ë?sêøV£.?z"wÞ7Ë?ïAæ̟£?wå°"»úi?Ã-KCŸ?wå°"»úiAGN4FGL J0505.6-1558¿ëg'ЛbÀ>n¾‰¬½À:"À';¯À<~iœ{Ì)@_ob¹]¯@MWoÈ?¿Ê™@Ù9?›¸œÇªÎ?ß¡'à'§b@šP¦`§`?ï'ɨU@¿áÉåX4¿ÜÉ þé7¿äæã>SLÙ¿Ô'üŸ"p¿äÂßäÆAGNbll3FGL J0505.5-1558TXS 0503-160?ïþfMo}?F"*B2?)›)<õ;¤?F"*B2?ïøX'ð
?OÖ®¦}ò?N¹¼Še?OÖ®¦}ò?ïóó7£8?lE®Ldu¶?X£'s
?lE®Ldu¶?ïýó%QT?HóxU¬?0f×*}ww?HóxU¬?ïýÝ
ë-¿?*æ*~¦ÿ\?1'Aš"?*æ*~¦ÿ\?ïà0{?r»Å×"Û´?o÷Ï«^ž?r»Å×"Û´?ïùîS¸Â\?]õjºìã?HF±ÜG3Í?]õjºìã?ïú°Ã+ä4?4gº(?E<ò-%¼?4gº(AGN4FGL J0505.6+6405¿â$^óÅ#@+kJfUŸoÀ:Í*ÀêÀ< {ÃW@+î¼@žß(Ã?¸¤³~:ž?Ň>£(ä@`ì>'Ï@	m8?ï³ÅP˜¿Éü.dAs¿çôß:šˆ¿â[?î¿êŽ›~¡¿ézNW‹ØAGNbcuTXS 0500+640?ïò"žÝȕ?]À0°"?[ºÂÅ %T?]À0°"?ïðtǨÄ?aÒ³{uø?_péyç/?aÒ³{uø?ï·7¡yYU?/Æ÷¿Œ?'2¦!(Ð?/Æ÷¿Œ?ïý'ÃzyÕ? ä¤|?3éâ?œŽ"? ä¤|?ïäÂt¯)y?dÚ>vôƒ>?k=‹+º¿i?dÚ>vôƒ>?ï¨IÇcE?Ú*r3=?…íŽzþ¸?Ú*r3=?îU¢Wi"?kÖ3±f?ª¥Ú‹…?kÖ3±f?ïø5ƒš~Ç?AÁ+ÿñ;?O)ñ®Ât?AÁ+ÿñ;AGN4FGL J0505.8+3322¿Õ)õžõp|ÀGlãËÀ:f÷ù¡A.À<­-@ l"
qË?þÄØý\·'?ÈÝ5:I|÷?Èϐa³'?ýÛs©EH@â²_¤¿ïÿ	*K-%?ïþY¢2ÅO¿£Gt!©·¹¿æ^ú+ª¨¶¿Ò"Üޒȿíñcºº{'AGNbcu2MASX J05054288+3321355?ïÝ՛}tu?ªP.––Yô?q20¹Ÿ?ªP.––Yô?ïߝ%¦i?x.Ä0ò?pr1`Î3™?x.Ä0ò?ïË8+`?vEí«¯½¾?zcöÿ¹#Ç?vEí«¯½¾?ïÊ0€®ï ?b¤½< •?zç¿¢Xä*?b¤½< •?ïǔ¿ÂÒ?wFžò_]¨?|5 7ýÏ"?wFžò_]¨?ïQÇ–9#? ¼ƒâúÀä?•Çð¨w˜? ¼ƒâúÀä?î2ËŸ?œçñÉ£‡?¦üÞä+­?œçñÉ£‡?îúÈV¬›:?ãœ#
è? Sz–3[?ãœ#
èAGN4FGL J0505.8-0419¿ïÁ‰ºJárÀ9f?x»Ó€À9·iþ¡[/À<œüûhÂ@«uÄ'aÄ@Ä#°ß0?µcl6	&?›m=ù"\ò?ä\õ8ü Ð@…ìiJF?ïïNlta¿Ö"vÅTÉ¿ç9.ŠWw¿â¿üò¿ì)ÞJ΅?µmôÐ!AGNfsrq3FGL J0505.3-0422S3 0503-04?ïý0
?(Î1-
\?7Þ~Cè@?(Î1-
\?ï÷NKp?Síue?QchÍLc+?Síue?ï¸>Š'Ú?ƒ—-ó÷Ä?ð,чV?ƒ—-ó÷Ä?ïþJtS !?½×ÀC'µ?+X¾áþQ?½×ÀC'µ?ïûjãsv?7ٜÁ– ?BTspèŸN?7ٜÁ– ?ïßSßÈtp?}Òì*›ï?pV?}Òì*›ï?ï§"â,¹?‡ý¿ð¿ª?†7yÊäm½?‡ý¿ð¿ª?ïüJÚ!|°?3SZ}ï¤?=©0yT¤?3SZ}ï¤AGN4FGL J0505.8-3817¿ïVmC—ÀB/@Ý?á—À:²'f™'À<ª; †ô@øáі¶?ÿ©òâáH?ÂâÍ)¾ë8?­#Ú¥¨p¢?ë)õœÏ®ÿ@	n»·¦Ÿç?ï¸Â‰|ëä¿ä"§Ös¿ä#ÁÛØ‹¿Ðð~BP1œ¿å¨Ñ F1¿ä3Û._"AGNbll1RXS J050559.9-382059?ïÿQ›öb•?ݜMn¨{?̂<p"c?ݜMn¨{?ïø"k²U¨?Oø(,`—?M®Q!ÅY?Oø(,`—?ïûy‡ø©Â?,A)cDvá?Bà°®žQ?,A)cDvá?ïýAÔ5?eN)(?5÷Iöހ?eN)(?ïÿúãØÏ?$‰ƒÊø±?RiMæ	?$‰ƒÊø±?ïÛñΗ…Ì?ƒjGÇÁ×p?r¹Ž?ƒjGÇÁ×p?ïü]ˆ
>â?BùÕÚ¢?=À:Å»û?BùÕÚ¢?ïù¯c&ã;?6óvîƒû?IBrÑmû?6óvîƒûAGN4FGL J0506.0+6113¿½¹ñ0ŒîC@(1\FRÀ9®ð©Jç…À<&¼ßï¿@@ ,µ?½Z@'.B2ªw?±"Ï?úT?Å^ïN­?àPž¨ø@Rïl_¿è'ýº*‰?¹SŠk©F`¿æ–!W=ª¿Ödéc±UM¿æ}º«bú¿ÁSæ.Ã7AGNbll3FGL J0505.9+6114RX J0505.9+6113?ïþX 0)Ç?ò͈Cß?*}ÿvµ&?ò͈Cß?ïñ¨ú±?\·Fý=B?\®Þx'yI?\·Fý=B?ïöÑ?UôV»bì?SüÕØ'?UôV»bì?ïò2oò^à?G_
È»t?[›°p?G_
È»t?ïý>r_ ª?0SK•¼Æ?6n0òd;?0SK•¼Æ?ïºÆ©¶áî?ˆ½ªéúºY?NU'?ˆ½ªéúºY?ïó"<s`?kÎÀñpr?Y»†ÉFQ;?kÎÀñpr?ïÔæ&:&l?gÉtÓ9—?uŒìÞÍAÈ?gÉtÓ9—AGN4FGL J0506.0-0357c¿ïgёhÙÄÀ9-DŽO¹À;{È0…ÙÉÀ<â¾|§ñK@  czΨD?þñìVuX?ÖÐ^ÚÖÑ?éµ°P•CÊ@
h¾/?ÿ-å^0´¿à­Îod;ê?ï"E¥%¾Ö?Í91d|'¿ßCµA?æJ¿ãð"aùð¿ïÿvä܎AGNbcu3FGL J0506.3-0357NVSS J050605-040152?ïÊ59.2?vý%d{p2?zåc†Š
Â?vý%d{p2?îg«4÷ƒ…?¯üK)Cý"?©…L¬<D»?¯üK)Cý"?ï!Ø ÚD?ŽÔ-AÁ;U?›ßDê,ét?ŽÔ-AÁ;U?êûÝ;ãc›?¢;ڞ™?Ä‹rq•?¢;ڞ™?ï$´D73ë?™>	ö¯çg?›iwzÑP—?™>	ö¯çg?è‰f‰T…œ?ËÌê0Ê?ÍÚeÚ­é?ËÌê0Ê?ìÇâíŒ?¨g¨J€d'?¹Àè—Gs¡?¨g¨J€d'?އ÷Ù®ˆ?¸ŠiQD™¢?à¼}"(¼?¸ŠiQD™¢0MIXED4FGL J0506.7-0857¿ÁÑ$øT\pÀ;O¯§"YÀ:3+y*ŽÀ<Y^¾Ò@"¾ì‡@Ÿ.cÀ™¹?¸3°ÜJÿƒûW2'?̦WB1(@/DŒ?ïÁ6á¾vs¿âØŸUd¿ây,Áÿê1¿å3+;-C¿ÞÚhH¿â¿ÚÖ­@•qlAGNbll2FGL J0506.5-09011WGA J0506.6-0857?ïþû­µÛ?!PØD}z?/àBWÀœu?!PØD}z?ïöË÷˜[	?TÚMÊ4?RhY_?TÚMÊ4?ïö ö…,û?W{[˗Ài?R¾¹,ê>?W{[˗Ài?ïü®a|È?'V%Î7ñ??Ž,4m?'V%Î7ñ?ïûz# …J?:_îZ¡v?Brðš?:_îZ¡v?ïß
Ã\Ã?sXLvhûŒ?pySz?sXLvhûŒ?ïõ¤×ª?e2=®N?U޵̺â?e2=®N?ïõºw­?DGEÂ<då?U‹%[±?DGEÂ<dåAGN4FGL J0506.9+0323¿ç9mþqpÂÀ5\ÓZ…‡"À:wO"¼
À<ZÀ2Š–Ç@ Ja·Õï¶?þÓۙï)ï?ÁÏo¹Ì?¤)JQ1öÈ?ãO]¶>–@Û̈́ؗ[¿è—¢KïÃ?ïé%=QD@¿ÛÈ*;<ìð¿âP7…¨K
¿ãJ™aj?Œ5¿28!AGNbll3FGL J0506.9+0321NVSS J050650+032401?ïý}…Ö‡û?$aš'æÊ?4Ò©¤j?$aš'æÊ?ïõ¬øy¬?WšÕ©9%?UЦ5ˆFç?WšÕ©9%?ïï§]&¡ª?a:w¹?`X¢ó{]}?a:w¹?ïìN& õü?LL‰†—?c±ÙÑ4›?LL‰†—?ïù³·Iz?C›sq8£?K1Ž
æp?C›sq8£?ïӜ"Òþ?'לsè?v1ö7vY9?'לsè?ïïÁ«¨Ý&?m·qÖ8È?`>TCå
C?m·qÖ8È?ï·diGR‹?qð"JP?'&å¢$»H?qð"JPAGN4FGL J0506.9-5435?¹å ²`×ÀBb‰üm¤HÀ9·zn['nÀ<D€bï@ }ëišù@?öb¼'«A?¸p°íOF?ÁÃÆé³ãG@ýöÀ¼R@èWº§¿ê°Öâz^¿Ó³(¶ØnÁ¿É1£:৿ÇLíCÌ¼¿ÕH[¬¿Õ<{ÜDdAGNbll3FGL J0506.9-54351ES 0505-546?ì«xÞQô-?Ó}éMØâ?º¤9
p^•?Ó}éMØâ?ïõ\óöÝB?SÍ!ݨ™?UFÞm*?SÍ!ݨ™?ïÓ<
cŽ?~Jçr©	‹?vaúÔñ1?~Jçr©	‹?ïóÊþý‡¼?AéF7?XjQçÇÜ?AéF7?ï³ç2Cõ?'ó¢ÀÚ?ƒ>­ï¢Ê?'ó¢ÀÚ?ïϼ<0Þ?'dЇìñÏ?x{¢ƒøò?'dЇìñÏ?ïSý7p&%?"¥Þün2à?•€Ye?"¥Þün2à?ïÑf+¥l®?g¼×uíùà?wLê7˜|÷?g¼×uíùàAGN4FGL J0507.4-3346¿ß#0Ÿb¹çÀA¦
á'6À:˜CÖ¥éÀ<'">iƒ@ ÈôíÓ,¸?ü¸<ÿ?½
uyÔ­A?å›G;]?ÓwE|Y@ãòóýé$¿îY»È˜Š¦?Ñ*²Æ'Ii¿ÚˆüéJ1¿Þf*]㋿ÐGòká%¿Õ¯?ˆ¬ŒAGNbcu1RXS J050727.6-334628?ïßǕF?¨¿æü¢9?p5'ù_Z?¨¿æü¢9?ï÷½Ru1Ÿ?PÈyî×F?P…[ݽ?PÈyî×F?ïëü¡ëf…?q~³há;?d^*–û.?q~³há;?ïý[/¦‹Å? Û#Bà×?5&ƒö³? Û#Bà×?ïûxÏ·?;H~ôW€!?BßCi1?;H~ôW€!?ïà_("ƒˆ?p'›ÖX9?o ×WÀˆR?p'›ÖX9?ïïóÊVi³?qIô÷S€%?`5yE>?qIô÷S€%?ï÷¾þX
-?D.Ü®4_?P'<­ÕÆ?D.Ü®4_AGN4FGL J0507.7-6104?îúǺqÞóÀAû‰?¯BxÀ9Ry§‹Ê¤À<¡V&}B@Ä*m @ö‡{‰ä?°ÅÜ~ײ•?²=Âno@@}ü…!=@ü!3Vn¢¿âMQâ É¿âò#žjº¿ç¤Ç+£¿åíuÿ‹í¿è˜b—¤ÌÔ¿ïÿÅ}M2¹AGNfsrq3FGL J0507.1-6102PMN J0507-6104?ïýf»ü?@
ÌGŒ\?4Ê''[5²?@
ÌGŒ\?ï÷!rý‰¿?RìØ1»?Q½3§1;?RìØ1»?ïÜ-˜Ð­?zM)
Ë[½?qÀiÚy™?zM)
Ë[½?ïü!2ÌþB?-rêkÀŒ?>öi'Ô/?-rêkÀŒ?ïüà¯$=?6}
}rÆ??Xü8=ø?6}
}rÆ?ïݞû˜I?r{K_Š¹?q0'p´{N?r{K_Š¹?ï·ÿ£í80?"ÅéIS\Ô?'ÈYø?"ÅéIS\Ô?ïïçtÿír?S¨e
?`‹Ͼ?S¨e
AGN4FGL J0507.9+4647¿å•Ykߪ©@vÊa¸¼À:	ÅDBO0À;I%Ü3@ú¦‡é˜à@á~4¹E?ÑÚØÞÓàg?ØÑÐAÌS*@准qž©@_Êe"Yi?£Pª"¹ús¿ã¹%¨05¿ä`‰þ#r¿éÿ}Ž¡¿ï÷x§±ŠQ¿ì)	ä…P6AGNbcuTXS 0503+466?îñdï÷Qä?¢6ÕÞ|J? é°þÓÀ?¢6ÕÞ|J?í†5N_?µÙ†9ÆJ?³ÏöVÙ·‰?µÙ†9ÆJ?íg]ÈÄ:¾? ¸·o'?´Å¸&\? ¸·o'?î~	Æ'l?‰×mš~?¯èdyp<?‰×mš~?émõq(.?½ùšÜËٙ?ÊK"*;_I?½ùšÜËٙ?Ûh•Ú11?ÑáGv¸?âKµ|'çh?ÑáGv¸?àŠTXXÿ?¹"ëEìoì?ÞëWOOÒ?¹"ëEìoì?àg°Dù%¾?³Ú… ^1?ß0Ÿv
´…?³Ú… ^1MIXED4FGL J0507.9+6737?è*M±í+@/ÉèPðÀ8vÖFÉ-À;›òâáH@!Š¿¨X¤?øž¥Ýtº½?ŸL¬^ ÒÑ? qÇÿ™¹á@ÔæŸê%@áY¡±ì?ïy¼NÐG¬?']$É8¿ÚþÜÇÔ¿Ë`À	Dø-¿Ð'¦ÂÌÊWƒ_—±AGNbll3FGL J0508.0+67361ES 0502+675?ïþ¯ÞT‰š?'"v¦~?%!ÝÅd?'"v¦~?ïò9›8*?\Öqš+Ð?[Ú˜KÉ?\Öqš+Ð?ïÁ–UõÞr?†«gïŸ×ï?4Õ}ã?†«gïŸ×ï?ïôP¯oï§?GQž‡Ïº?W^ ù¥?GQž‡Ïº?ïýG"EÜ?18™FªE?5Æïô£¨š?18™FªE?ïÁV¥0Ú?ƒŽPÀ·?T­ƒÒL?ƒŽPÀ·?ïµ\ã°¿?‰>'ªf[Ú?'ºhä4F?‰>'ªf[Ú?ïïÀ{ÊjŒ?Uï'A0¯?`?"ÚĘ?Uï'A0¯AGN4FGL J0508.2-1937?ëŠï®µÀ?2×@ÄnÀ;*í"1{À<µrþ$]­@xC¬':×@åPäôá¿?Êú8À»Çl?ØHC{)ìã@C"¡@µÚ,†Æ®¿ïÝ7~ŽÒ?ïÔ£"`š¿àé.AÜÄ<¿åºðáÿäÒ¿íøwÀ«×4¿ïÿý±q&´AGNfsrq3FGL J0508.2-1936PMN J0508-1936?ïÆ@Ssß?y+LW#=?|ßøo³,@?y+LW#=?ïÉÑO$?Ãl—Q¨?{@q߉ô?Ãl—Q¨?î£{e"œ»?'¨îÁ×4â?¥ÈI§¶4Q?'¨îÁ×4â?ïn¡è–?s¼-òDi0?'+Üh%wA?s¼-òDi0?ïyt%ä?'™Jßå<â?Ñ{[‹¯?'™Jßå<â?îÍß4¿‹'?«¶ï(úó?£"²Oyä?«¶ï(úó?ꣵ1®+€?¯O@pb²Š?Åq+9GR?¯O@pb²Š?ì`»£üì?ªA¶Hoé?¿,ú"àž?ªA¶HoéAGN4FGL J0508.2+5211?íû €~@5#ŸAyGÀ:ÀÞ­ŸàÛÀ<4p¿…¼m@ 
z?â@I´˜c9?Ō[ØîÄ?¨ÉÀ°3å?äù]ÿºŠÖ@mà0ù¥?é"ó1»cï?ïøø²<(¿Õð¡¾+IZ¿æ
gAؒ~¿ç®±Ž'å"?·ôƐó'ÄAGNbcuNVSS J050809+521256?ïýº«è?)wÊìNa7?2/KKðl?)wÊìNa7?ïëQr8§?hÓÉÞ^YM?d®·9c?hÓÉÞ^YM?ïè4ἧ?oa•¯י?gÿË£1g?oa•¯י?ïå¶
v=Ò?Qo9C¤ŒÀ?jIònEMª?Qo9C¤ŒÀ?ïúF‹2VG?AÓæ~E?FåÒëâ—S?AÓæ~E?ïj¯¡BÛG?›\iHª$?'ªރÏ?›\iHª$?ïÌÛµóÂZ?€'LŽ_'þ?y'$ê¡ó%?€'LŽ_'þ?ïœg¾'•?xB4Œà\Ñ?ˆæn ê½?xB4Œà\ÑAGN4FGL J0509.1+1943?â¨)ƒ Í¯À'ý¼#1]pÀ:	ã<zڒÀ;Ÿæ·Yž@E	¬§@†'QúŸ?Ο¹ï$'?¸F7qÜ;U?èì&>ƒ@ícíbt¿êÁ¢Âi¿ÝXl¾U¼¿ècya•Ç'¿èêŒeÔp/¿ïû'Á^Á?ÐC	Ÿ»òŠAGNbcuTXS 0506+196?ïú,ì>¤x?Bs1.Á†?GLOˆÒbã?Bs1.Á†?ïíRÆÌW²?ië?˜`"n?b­9+n9?ië?˜`"n?ïZv6Ï0;?‰¡ìÛRO?"±9)‰"¨?‰¡ìÛRO?ïç	 åþ¢?RÁ±%Õd9?höߤ?RÁ±%Õd9?ïùˆ/l‡Æ?J´ô	må?IßCCžX?J´ô	må?ï˜ù_£˜?'ñËþ©eU?‰Á¼ÝÈEõ?'ñËþ©eU?í¸xA…0?£l/Jò?²<=óÖ{ø?£l/Jò?îË$»˜"X?"SžeíV?£M´D¾ì|?"SžeíVAGN4FGL J0509.2+5550¿ïÎ"þæ-@"Ÿhß½jYÀ:.¶ÁȍÀ<~'­N@;2'D"@˜<ÿ?ÅùԂM͓?¿í½‡?ù7ýÒÿõ@<!í%?ÞþáEª¯¿×*&ʺϿå$u*Nˆ#¿ÜÞ硺Or¿ç¶?A´U¿ïþ±`à•'AGNbcuGB6 J0509+5546?ïôÐgó›?Nž—x3Ź?V_0Yl?Nž—x3Ź?ïÝùz!Pª?oCY‰È?qBäXë?oCY‰È?ïà—¢s‡â?s
XžHË6?oh]VÞ6>?s
XžHË6?ï¤á"OÊæ?`ÜæËÁ¬?†Ç›2ì~}?`ÜæËÁ¬?X±?ˆ´r¾Û¤?‡•_"ëz?ˆ´r¾Û¤?ïQY]ƒ-?˜+íùÖ
Ý?•ÝÔÍpbs?˜+íùÖ
Ý?îó_EŠÎ¦?V
Ñðe=? Ê¤¿`ª?V
Ñðe=?îҔ??ŽìÌJ?¯âÖ»˜Yï?ŽìÌJAGN4FGL J0509.3-2917?áu…tï	À@ïßã*dÀ;	üȽÀ<»ÃlѺr@ùeä@|ÍT¤?ǼƒDÃ~¿n$M$;—²?¬fóªNN?þ‰ð¯*%¿ì–ŸV¿ÑΗÝ×·¿æ
|?ì¿Þ;	ÛØ¿à8èê9Å¿ïó/lÕqAGNbcuNVSS J050927-291339?ïýڏ"CU?"'X"<?1+ƒ§-§?"'X"<?ïõ2¶Øç?Y'¢ƒhÏ?Uš'ö;øÖ?Y'¢ƒhÏ?ïéz€àÌD?VÑägáÏ2?f…K.»v?VÑägáÏ2?ïúGRé ²?/Ä3°Gá?Fâ´æÆÁ?/Ä3°Gá?ïüàÝ"?0vÔîek?8û—š0iý?0vÔîek?ïØ;]y,è?v¤ð8"zQ?sâQB¹ 7?v¤ð8"zQ?ïÜÍYïÇ?t½…ý‰š?q™tÎ8¨­?t½…ý‰š?ïÛýŒ–?c§>>E]G?rpA€XÎ?c§>>E]GAGN4FGL J0509.4+1012¿îì"ÑÍMâÀ1>°ÙQ?ŽÀ9YµÂÅÀ;î:Ç|*ô@s·ìj÷Æ@×~¶ß%?³<ƒd?¹1¨C«{n@:$¾ü*@Š_[^?ïû‹[é4â¿àAR—M¿ædÊðSº'¿æ†Å~ð¡¿ç'uÞ©¿çBž
A¢bAGNfsrq3FGL J0509.3+1012PKS 0506+101?ïþèk
êú?§dW—˜?!yR0*‹®?§dW—˜?ïôôÀÿ¦?X=Ŭ±?V}½<ƒ`?X=Ŭ±?ïèC4Õl%?q¡ã*Œd‹?g¼ËGp'É?q¡ã*Œd‹?ïú_—•2'?1EYËûp6?F¢pþ‹?1EYËûp6?ïþÅxÂ?"jN®¾?#¨{îòq?"jN®¾?ïØOA±¦+?wëb0A&i?sØ_ßV·?wëb0A&i?ï¹sõ×CZ?ƒZžn®÷?£–å·Ž?ƒZžn®÷?ïv^?N€²pö'?aq^£Œª"?N€²pö'AGN4FGL J0509.4+0542?êP1Š€fÀ3¡zÌNøŒÀ7K(û¡ÌnÀ:î
N@êÙð¡¾+?ÿîȺïT·?–~1xï?ªŸþ…+£@H×°´h@'í~<Q¿Á@WH'>V¿Û R›X`"¿âÚ>û=y¿ß,J
æ
¿å#ªß½s¿áͽ¸‡ÆAGNbll3FGL J0509.4+0541TXS 0506+056?ïûO›b‹T?A|v·ï?BÁ'¸Y?A|v·ï?ïõܱØeî?T=x*Ì?TFœe1£2?T=x*Ì?ïÈ£'–Æ?'ub¢±K?{®6Ã\?'ub¢±K?ïÿ¢%jƒé>þè¿U2V?v–û8>þè¿U2V?ïý®bdµH?+£æiªŸ?2Œì'Äj™?+£æiªŸ?ïÒ`c~;?ù)A'ÚM?vÿO´Óƹ?ù)A'ÚM?ïÒVè«5ß?ƒ4Ýb¬?vԋ¿¸+?ƒ4Ýb¬?ïÿvñV¢'?	I'Eæn£?!ÍQlj?	I'Eæn£AGN4FGL J0509.6+8425¿îA‰Å¨ã@8ŸB»früÀ:ö,ÂãÀ<‹2§òø±@Ö ‰ÍÉ¢@`ù$C¬'?Å^I·Y¿³árÌ%]?ìá¼]"Ùç@ËîX^¼?ïúwàŒGL¿ç³ï†¿é¯Pð³[â¿ãƁŽàØó¿ð?ðAGNbllS5 0454+84?ïÙѸÍo?¥*\»eóÚ?s#´jþ?¥*\»eóÚ?ïå_·g«?{Hbé[B?j H•´~?{Hbé[B?ï&þ
EZ?"Ô5?› =œŸ†¹?"Ô5?ïæ
pUþd?VxDŠH˜Ë?iò~›ô?VxDŠH˜Ë?ïåúØù«Ó?rM'S=®#?j'\Ü?rM'S=®#?ï6UÔjG?¤»"€üÁf?™=@KM?¤»"€üÁf?ïcý `?'ør¢ü?"@ZG¦?'ør¢ü?în‰s[Â?›ÏÁ—…
?©Gf6Žß?›ÏÁ—…
AGN4FGL J0509.6-0402¿î!kNqlÀ8k™¡ýjÀ:'Ò¬áÀ<ZÆã~¿ù@ &|'²wa@h_dêed?Áb¥üÿD™¿'=<Ÿ/?ÒïœePç¤@"‡®‹?ï÷z>Š¿ã8Õ3£›¿çdú Å‡ß¿Ö—-ƒ›Ö`¿ßÖ­3ªQ¿Þ³Ë>WS¤AGNbll3FGL J0509.7-04001H 0506-039?ïü©¶óÁ?,ÜUW¼6Z?:²F‹Mê?,ÜUW¼6Z?ï÷¯:ì?TÙ~Â@í\?QõæÞH?TÙ~Â@í\?ïõ·?
Ç?`*ÖRê?U'23ƒ6?`*ÖRê?ïøx­÷Ûª?0Ž	àCZ?NG£:ä?0Ž	àCZ?ïû¶:ÚÁ?6Ž¼ŽÕA¶?A'.bn€?6Ž¼ŽÕA¶?ïܙî˜Ï?|'Ï»Ýæ?q³r ÀÜ'?|'Ï»Ýæ?ï÷þym)N?dìT —ïÞ?P
PŽéÑ?dìT —ïÞ?ï㌠¬•A?Wğ	x­C?lsßw&®'?Wğ	x­CAGN4FGL J0509.9-6417¿â"ÄoÀA˜>}QÀ:N°÷"0|À<"ê"]ðv@ Eúأŗ?þ-Aª?µ¾ S¿ƒ'ëÆ&d?Ð`¼ÃÀ3·@	Ý
$¿á¨†Ò¸©¿ã·S½v¿à*®"Óa<¿Ù‹z‡…šß¿ÚoUã·J¿ÜM8'}sHAGNbcu3FGL J0509.7-6418RBS 0625?ïÿ>iQ?
>ø¸»
?=|¼Ü¤Î?
>ø¸»
?ïöûX•1D?Sѧëª})?R	N¿Ÿøa?Sѧëª})?ïø?Pð)ì?eˆbW=Ÿ?O»æHØÕ?eˆbW=Ÿ?ïÿ+ŒÔAê?£ìÊ¢YS?Ži 	?£ìÊ¢YS?ïÿÜe­?O…$3v6?<T¬,?O…$3v6?ïãŸL¿~ä?o9€î"«?l`³+ãt?o9€î"«?ïü˜¼qWS?VÇmª¹å²?;:'ÛÄ¥?VÇmª¹å²?ïþs]"y?#)ۉówþ?.¸Í(è?#)ۉówþAGN4FGL J0510.0+1800¿êÈÛ?pÀ)p—AЅÀ7÷uôxãAÀ;F­)¬@žp•@­@ÅÂíP?žs_Yhj?·«#Ú¥¨q@]¢r†/@xkv›"?¡ˆeûÖ~¿às-õÐú¿âKL.¬»µ¿â']ÂS¿æâZh+b"¿ê½4D«+AGNfsrq3FGL J0510.0+1802PKS 0507+17?ïûbuQL	?@¤"cî?Bv)ºs&?@¤"cî?ïïÇû¬Ã?n6¥µ²$?`8Òl¿?n6¥µ²$?ïΩ™Ÿn?€ãk"L€î?x«32O
$?€ãk"L€î?ïÿ¤¾™`í>ü—£5Š$"?Ðg2O§>ü—£5Š$"?ïü]­ˆ?=ÌÐÍyâØ?=˜¹éc?=ÌÐÍyâØ?ïÄ]¼b‹)?‹F»{JŒ?}Ñ!ÑzP?‹F»{JŒ?ïÁìÎÂ<È?…³ç£'Á¹?	˜–¢‹á?…³ç£'Á¹?ïÿCò?šl?"YàÙ»P?¾äá?"YàÙ»PAGN4FGL J0510.4-1809?å­>kÀ>05z5PDÀ:¢ÏîÀ<œÀ<uªŠ'¥a@%ònZ@5ÚBU?DZ¼»‡«?ÀêB> ?ôE;ÞÓ_Ž@
åð¦p‹¿àsco;!>¿×!˜ r¼5¿èà<K	鎿çŸÌäu¿ãC‡^ƒ˜ü¿ïÿšÏúAGNbcuCRATES J051015.50-181227.8?íTë•Ëêá?иF2i^¾?µX£R|ù?иF2i^¾?ïölÛg"?R‹›&|—?S'ÓÝýì"?R‹›&|—?ïï®0eµ?WdGž˜?`øQÀ|t?WdGž˜?ïý®–¥§?Րå:?2Í`%f?Րå:?ïýáJïM¼?UvîE+Ñë?0õ©K{œ?UvîE+Ñë?ïÙÖã"?€6ñ3£Œ?ssn$âj?€6ñ3£Œ?ïÚñCµÈ‹?u,º³ñ?r‡^,¾Ê?u,º³ñ?ïó–¬Ä?Kœù?¨¡ì?XzÒ£¸@Î?Kœù?¨¡ìAGN4FGL J0511.4-6804¿åX…à19ÀA%×ý'w>À:Ï&رÝÀ<.šLGp@p¦d]þ@ºV€?U€?ÅãæÄŗN¿mÜ^y?¡'G=VM@'º¹Në ?ð¿èZ,fWѿ듦¹Ù«¿ß|"¦Ò¿ÒŒ\š4Ê¿ïø×aütAGNbcuPMN J0511-6806?ïþ™‡]½? gFÆf6"?&g‹÷ˆ}? gFÆf6"?ïö–#1LB?Ub{…gt?RÓ¹¥¦‹Ñ?Ub{…gt?ïãö†HrÏ?q´p\và?l	yŽQàõ?q´p\và?ïÿCø°Þã?W£ŽBˆÐ?€ì.Ö¦€?W£ŽBˆÐ?ïýÍ+¨‹‹?9nËæÇ7Ã?1–¤¶ƒà?9nËæÇ7Ã?ïâq«­²?p->p?mŽT2±~û?p->p?ïɍ¡$
¸?€¨m\¥w?{9/qhÀ6?€¨m\¥w?ïücç
ÉJ?3Èd#?<àÉ=ktÌ?3Èd#AGN4FGL J0512.8+4041¿ïÿúfþ†?íJf@%ßãÀ9N™û¿(ŸÀ;Å(wŽ'@0—²Ž³@TZDïô?µØJÀ~Æì?©ÚˆÍ¢
?ñËÏÇSH@Ñá»Fg˜?É"üÚ0¹¿ç¡Ìþ¿á¹	ÁŸÈ¿åF]É^ٿ༰À&Ì¿ìaU_Ø؟AGNbcu3FGL J0512.9+4038B3 0509+406?ïüÏ9õ«O?.†¯Ëì>?9†0i¼…1?.†¯Ëì>?ïçAQÂü?yWçƒQm?h¾ïµ;|?yWçƒQm?ïçýÈBN"?oRoÄ?h7ÿ©ûˆ?oRoÄ?ïü,v*ª?&̜"¥d[?;œ/áfO?&̜"¥d[?ïùw®ÉgÏ?A®o¤Mî?J!D'÷'"?A®o¤Mî?ï@n¾`†?¥©ñ­6Av?—ò(F³';?¥©ñ­6Av?ïׄuÊK?€ÖŠÇ¶æÆ?t=ý¶¬~i?€ÖŠÇ¶æÆ?ï÷ƒnÆ?AUCôž?Qþùôpí?AUCôžAGN4FGL J0513.9-3746¿ï¼ÜôQÀA[¾<Q‡À:ûÏ[óEÝÀ<~>TÏe.@)aIñæ@>"DÎf*?ÕzOÇã?ÞóÞ>d>Ä?ü4E]c@3ÝKue?îñïÁ™gð¿ÂtlùÓk"¿å6Aü$¿ïÿî—ø¯ª?ïþ{¿ïÿ7Mt'AGNbllNVSS J051404-374607?ïû¬|ÜZÆ?[99"'Æ%?ANc6Í?[99"'Æ%?ïõóS8%$?Sˆ{£µ2?TY×-—?Sˆ{£µ2?îÖDي¹?–©¸*eL?¢›²ióYl?–©¸*eL?ïþËJtK	?!gþnS?#KTt2Z ?!gþnS?ïöÅP£þÅ?ZÈè¶À…?Ru^6Ñ'A?ZÈè¶À…?ïÌä«v÷ê?"Üa=¨D<?yªb®µ?"Üa=¨D<?íNäü2YÞ?¤á>qE`´?µˆØI
?¤á>qE`´?ïíg«¤¢Ñ?eÍ@­÷¢?b˜Ty™¾ì?eÍ@­÷¢AGN4FGL J0514.5+6247¿èŠOXûN@+š™0¾
íÀ:£>ºOò‡À<uÌÿøsD@µø/°@"EœÂC?ÂnʸöV3?»ñ'Ž»F?ú|ÌQ#ß@€ýêQ¿æj8î^
?ìšÏú¿äW­Ñ_Å¿ÜXGŸ{ÛÄ¿â^zd¿ãœg¿¬Ó³AGNbcuGB6 J0514+6244?ïc¿§—«z?À³…
›t?"ˆ1ú²?À³…
›t?ïî˜÷³*d?eèû"Óç"?ag$ú#à?eèû"Óç"?ïõû~ÞNÍ?c´›ø-?T	@¢¶'?c´›ø-?ïìŸù¸›Æ?DäâÁžm?c`4&j#?DäâÁžm?ïý'Ð]Ã?1i.ˆ^Ys?3é~•q¸í?1i.ˆ^Ys?襤ÌÊëÃ?Ž¯õÇ/
'?†ÖÌ¿†Ÿ3?Ž¯õÇ/
'?ïïl׉?s™²KÊ·Q?`çå¦fGd?s™²KÊ·Q?ï¡t2ƕ•?tð¸}+Ç?‡¢óU9Ò»?tð¸}+ÇAGN4FGL J0515.5-0125¿ÆÔQ˔À5â]B¡À:š¶ŽœæUÀ<^@îݘÍ@s–ñ?ùüÜÊpÑú?ÔKa}H€!?Ô.á_+Â?þl˜å>³š@‹ö~•?ïû¢}˜Ý¿è¯L¾õsµ¿á§?¿³‰°¿ÒÇÜ£¦¿åŽé<o¿æÞÛB0|AGNbcu3FGL J0515.5-0123NVSS J051536-012427?ïú2Yª§o??6!~B¹®?G6˜X±??6!~B¹®?ïõU!ù½?V{½´­¦?UU»ßAÖþ?V{½´­¦?ï·ù
îE˜?ƒ.bïÆ?'½5PQü?ƒ.bïÆ?ïåºò"ÂG?GñÎçGœ?jE
IÃY8?GñÎçGœ?ï÷yl02€?PV®…œÂ?Q
'¢Z¯5?PV®…œÂ?ïÖ ™%?v°Ôi¹?tð/àeÙj?v°Ôi¹?說VO6?‰ñ •˜?†Wªˆj¢T?‰ñ •˜?ﳆ6)K˜?l×>"}ß?ƒrm%?l×>"}ßAGN4FGL J0515.6-4556?íeQ"LèÀA°K	éÎÀ8Äb\ìj!À;ý'æ÷ñ@ƒ)[Cµ@%AÁÇ?§´Èbô…½?©»Ôàu(Õ@$x]ï"@ØëpR#?!HW»0¿áÜ_|gY«¿æL8½¶¯¿äR½ú¡ò¿éwomv% ¿ëQ­DqIAGNfsrq3FGL J0515.3-4557PKS 0514-459?ïâ
òªàq?­žïE§ç×?mõ
FÚ?­žïE§ç×?ïø[ (˜¿?O-œ¿Gi°?N'÷‹'?O-œ¿Gi°?ïä>ØFÂK?tr_W¥@?kÁ'‡ÃUB?tr_W¥@?ïÿçcHq*>â ¨z9æ>蜚,jp‹>â ¨z9æ?ïý
=ú?3p@7tš"?7Ǭ')mC?3p@7tš"?ïÝ|…6¶ ?~ÎoÍÿ*?qA½_Õ|A?~ÎoÍÿ*?ïЎM`0?6'f	>V?w¸ÙVÇ,½?6'f	>V?ïÿç¥n1>æÅ-é>èýoÊG>æÅ-éAGN4FGL J0515.8+1527?æ;‰Ö­÷À*!ÅXdEÀ8ådÍßòCÀ;¶_"ÊÕ|@ É®ŠA?ýµØy©9J?®èO_8Ê¢?´ß="u@ÇiÃèø|@
¸÷f©WR¿ç8ôõ
¿Ø¨ÆÞ \A¿Øc¾ÁF[Ú¿ÝbßÆú{¿áÚaàŨ¿×¥Â¼þx–AGNbll3FGL J0515.8+1526GB6 J0515+1527?ïþòó8Wœ?"ÅM€? ÐÏ:6Cö?"ÅM€?ïõì?Œ?W:È#Õ?UÞ'y©×°?W:È#Õ?ïï>£n?m÷ö\©?`áàÚÂA?m÷ö\©?ïóœÊ¦ß?DLöÅCŠ?XÆjás?DLöÅCŠ?ïüù,sÔ?0VIU@Ñ?86œ1—Z?0VIU@Ñ?ïД¯œ\º?|çƒ_×ê?wµ¨FoJó?|çƒ_×ê?ïêÊÕ…¤?s 9í¢[?e5+˜£É?s 9í¢[?ïÚ<êl?e'lYêŠ?rኳõ}Ø?e'lYêŠAGN4FGL J0515.9+0537¿€–=¶pGAÀ2Iâ%úeŒÀ:÷ÒîNý"À<AÍ¡Þâ@Sõ±G‹/@'l6Kì?ÓaŽºú½¿",ß5N?ÂgBÚE0a?û»‡ëqR©¿å;66ó²¿å_"û-¿ã4íþÖ	¿àŸ=è˜Û.¿ã€´ÆEÊ¿ïê¶YFmAGNbcuTXS 0513+054?ïýÃЭ_¨?$',Á•¾C?1á|93%?$',Á•¾C?ïòMoŸu&?_ÕO#ET?[e ܒ"L?_ÕO#ET?ïçÏ…®?l!‹Ì?žÒ?h0ú±ÿò_?l!‹Ì?žÒ?ïñÕҍ4?A5õ–(Ñ?\UÐh¤|?A5õ–(Ñ?ïüP'2B?:SÿcFÏ?={}ä@¿?:SÿcFÏ?ïÏ)ïpCh?|-¡Hn•?xkVü""?|-¡Hn•?ïÑÝy²q?€ƒ	±Ååq?wC;—on?€ƒ	±Ååq?ï‹Ú¡5x?~h¥	$·?	WÄAuÝ?~h¥	$·AGN4FGL J0516.1-7240?Ó|T…¤€dÀ@kè^9qÀ:gÝDUGÀ<2Ô\.Õ@|<uQ:Û@ü
éÿ
?Ãw©Å5Ô£?³'Þ
øø?ðG™ò"í?þ.zœ~Ph¿â5N`¶#=¿çv-NäH¿ç|U†DR?¿è@¦¹<Í¿ïÉéÍ³}¿ï	AÈ!laAGNbcuPKS 0517-726?ïæÕÃÛ%o?›š—y0?i*<ü™0?›š—y0?ïÙqLÊÌ?'s0Zƒ?sGYñ¼?'s0Zƒ?ï¯V>n{?}®ç9*³#?"*¾"Ñ@?}®ç9*³#?﹧:/ëo?hÁ¦á‰?–1}ü8?hÁ¦á‰?ïߟÐóօ?q9?­ªŸ?p0†½¸?q9?­ªŸ?ï^½RäÜí?¢r×ê¶bj?"(UŸôÆt?¢r×ê¶bj?ïi¤ÓxQd?Œiïð®Í_?'Ëe™ŒÙm?Œiïð®Í_?í>zÝýÝÍ?£—RoE	?¶)ìø–?£—RoE	AGN4FGL J0516.4+7350?í~"$Ï1@3Åf'|EÌÀ:~…AÀ<uV=ú6'@ I«w?ü΍+Í
d?¶{iضºè?°õØ^ÑF¯?ù-6´Çó?øòuJ×?ïÿ2z¦K¿çiÊ¿+y€¿Ï¡ªŠ,¿¿Ü=›{?¼¿Ý ¡€mΐ¿àÚÞrç~)AGNbll3FGL J0516.3+7351GB6 J0516+7350?ïübËH¶?2ž'ÚPß??tçÿƒîõ?2ž'ÚPß?ïÎÂwM-I?{äãm¯?xžÄ{Ås<?{äãm¯?ïÚͧ¤Zy?w±®¾bßp?r™,)O…?w±®¾bßp?îí'mçuV?'¨ÍiÛ+?¡&Ù"d'¢?'¨ÍiÛ+?ïõ…ßí)Ó?R
Õ­¨d?Tô?ºx‰ñ?R
Õ­¨d?ï_$lŠ²?¨¦b®4¬?Ÿ´uÞEÉ?¨¦b®4¬?ïÎ¥7Ã?€E}O·?x­d&&t?€E}O·?ì}™™U?£"…½òþà?¿ó35Y?£"…½òþàAGN4FGL J0516.7-6207?Í y'W'ÀAaÅ.rÚÀ8šq
"=À;Àâf'@·ut@Ù ¡`7?¢[_LA?¨'K‰Á4@!Àoz@h²ŠMÈ?àÀgc¼gû¿ß}¡ku¿ãŽ¶aP|ð¿à˜ö«:¬¿æ䁦ާ¿åó
ƒç€­AGNbll3FGL J0516.7-6207PKS 0516-621?ïþ±"WØ{?ò_kýC¤?$æÆÁ'>?ò_kýC¤?ï÷‰Uöùé?Sçك—Œ?PíTQDüî?Sçك—Œ?ïò†ø&å?cë·ÊåH?Zó×üteô?cë·ÊåH?ïÿöÍ?lr'Áö?žuDOc3?lr'Áö?ïþfá¥;?iyåÆ"o?'éŽ/±ñ«?iyåÆ"o?ïÜy#òo?~öYÅ
?qÃm÷Ù¿?~öYÅ
?ïì…:W?jø=ì-:û?czþýå1<?jø=ì-:û?ïþˆÛu ?ãòTaÜ?'rEéê±?ãòTaÜAGN4FGL J0516.8-0509?æRʊɼÀ7YfYÑ,®À:`œøÉ«À;÷À¬-@ÆÎi/œ@C¼Œã©?ÇÝCýÛ¸x?Ù)x¸.@H/yjO)@	†qÀ?ÆxÌ$ý»¿ãu"FK=ì¿ê{>º¥Ù¿îÞwëÉè¿ïÿ¤?åÉ?æ2ËŸAGNbcuPMN J0517-0520?ïøÅþâõ?MºÝ¤jo?LëóxD½?MºÝ¤jo?ï瘫̼?q¦Oç…I?hãg…­£ò?q¦Oç…I?ïú{º>2?Y|Ú,m?Ÿ`°Šp¯?Y|Ú,m?ïÕL	Cý?_꧷•1C?uYû%P±?_꧷•1C?ïô1ÊèF?^4ä}»?WÖz­"Ÿ?^4ä}»?ïKTõzÀæ?¤LÜmýÕ?–•aUÏM,?¤LÜmýÕ?푻ŠçM?¤ýÆ
É-?³r#®¼Þœ?¤ýÆ
É-?íÙÐܯvƒ? ¶/¯0Š?±1y¨dç? ¶/¯0ŠAGN4FGL J0517.5+0858?×)ùë¥À01w…r›(À;e DC%ïÀ<ì&qƒÐÚ@!F€ÞaÊ ?ý痾Ή?Û
úD5ë?ïÿÜ>Y×ã@ÝK 'ß@M T3^¿évá]ÓoÔ¿îí0º²îÕ?àÖýr‡?¹¸ÁÝõ-¿ê²÷¤ëá¿ï÷ÇLZK¦AGNfsrq3FGL J0517.5+0902PMN J0517+0858?ï;‹_«G}?¡(08Á`?˜Ž"¾zT?¡(08Á`?ï|¹åûƒ*?žµÐ_Vç?hÃ=þË?žµÐ_Vç?íÕLöò ?ŸónzÜë?±UŸHnü?ŸónzÜë?ìųùõ­t?¤´ÏìA%G?¹Ò`0R"^?¤´ÏìA%G?í=~X?ºy "3DÀ?¶$÷€?ºy "3DÀ?îsGû
Ê:?º]/AGYA?¨Ë€SnßS?º]/AGYA?êÈɝmc±?³^˜6É?ÄÜيJq=?³^˜6É?ä¾XHU¯?‰¤'«ÚS?փOËoT¢?‰¤'«ÚSAGN4FGL J0517.7-1758?óâ)À<ƒ…@FA-À;SPßìdÀ<n"d¦rÆ@ÙZ.Ÿ¦@?û˜'3?ÓààHŠ?èö'¤‰·¤@
;&wºL@JE)B¿àÔMà½?½t˜j¾e¿ã«Þj®õ¿îwàmò¿³Ï?Bàû-¿ïÿÂ"NßaAGNbcuPMN J0517-1756?ïø¶ê&=Æ?SHžBØ:?M$V³C¾Ô?SHžBØ:?ïñ!žhé×?\l/lîڃ?]¼Âжò‰?\l/lîڃ?î­é(e?–T]×b?¥!oÊí´?–T]×b?ïéŒçb,ù?V´ò§.-?fsÅ®~c?V´ò§.-?ïäÊÞÍì?uãDۖ²?k5"OM?uãDۖ²?Ö?<V?"û=¾öw ?‰ØŠ}ïZq?"û=¾öw ?ìµqhšjœ?¨'"
»?ºTt»,«?¨'"
»?î÷)‹ÙVb?•Ì'ˆ? gD"gá?•Ì'ˆAGN4FGL J0519.0+0851?äZ6¤¤1À/ß-@ªëÀ9:2áԛÎÀ; ˆp|iÞ@ûPæ¢`è@Œz¤áÌ8?¹óô®é?Éme^(ªC@h@µKü­»?Ез=¿áIéXÎG¿èÐn**¿èƇ~9ö¿íÕç]qË?¤7ÀvõAGNbcu3FGL J0519.5+0852TXS 0516+087?íáG¼"Tí?°—àÃ
?°õÂ÷e?°—àÃ
?ïJž]½d>? ­… ö!?–¬4F›ªG? ­… ö!?î7{CÔ?œU¶öËÐ?¬
¹?œU¶öËÐ?îÄ΄:•[?'®™ídºo?£³¹ÂõW?'®™ídºo?âŒóe_M?É5€_IÖ?ÛÈæ5Ag?É5€_IÖ?æ"?ka??ÌÁ‰U\[~?Òׁ)=ï'?ÌÁ‰U\[~?âz¸ÂÌZ?¹"Àâ×ÒÅ?Û
ŽzgáL?¹"Àâ×ÒÅ?ä&çE§‡¡?¶)g˜Å¨#?ײ1t°ð½?¶)g˜Å¨#AGN4FGL J0519.6+2744¿×ô ý ÞÀÍW¼w¯À:œŒ" ÚÀ;ætxwàâ@  àBöIÉ?ë6™ŸxÖ«?éýáí›N?æ‰=–c"4?ü"§—‰!@ùQê™¿æT~<Fl¿êöDà"º¿ä)%}½ðç¿Ôr;†¾Ì¿á$ùê<I\¿ïþ«6z'AGNbcu3FGL J0519.3+27464C +27.15?ïõd€³Ç?j&ný*aú?U6þmÓrü?j&ný*aú?ïðÂF¥Å'?bt9"—{?^{rÄòþ…?bt9"—{?îÎŒIœN?—K~Ï+n?£=ùð"?—K~Ï+n?ïû"EO?ƒ?2õÞÉÃB"?Cv뚃8?2õÞÉÃB"?ïøӑôÿ?` b£É«S?L±¸¶?` b£É«S?ï®Â"µ?Œ(7@Xì?"{ˆí¦–?Œ(7@Xì?î¬5€ÈðÓ? EÎíî˜j?¥<§öàŽÏ? EÎíî˜j?ïøÖÍÎ÷Â?Lp£16?L¤Éz¥Ñ³?Lp£16AGN4FGL J0519.6-4544?ï4˜H¿?#ÀAUa=1¹¶À:6Ô;VdÀ<~¡ÆŽÅ@QmPæL{@'@œ¨AÓ?·óTKâÿª¾ÜŸ'Íú?ò•ôÿý²?ÿÓqíLa¿ÞÍ–%œ¿éŠŸ䍿æwé`J¿åÌQ¢_¿å4јäh¿ÕV¢ƒÎTAGNrdg3FGL J0519.2-4542Pictor A?ïúêÀ¹Õ5?3WÆ憎?DTý^Á
?3WÆ憎?ïðéüÕËp?^+ªmá?^,"¡î·?^+ªmá?ïÙøÔ?rîêžaÜì?söYa
î?rîêžaÜì?ï腛ǘ?M?EYVxÍ?gzcùŘl?M?EYVxÍ?ïñ³œ­¨Î?N'?Ç»÷Û?\˜Æm´¤½?N'?Ç»÷Û?ï¹kcÒ@?ˆr&rŒbÅ?¥'6cµû?ˆr&rŒbÅ?ï¸|ÒÓ:ê?'Œ¶7Ü#¦?àËCJ+—?'Œ¶7Ü#¦?îí£¶A߸?ô¾I¦?¡%Ĝ½ë|?ô¾I¦AGN4FGL J0521.3-1734?íû[ؐF×À;Ž~bÜn+À:dál—À<>'(ŒD@¢ÁÙ©ª@É%x_?Á¡??Ûã?ϘiƒQX¸@
Ь¥åØ7?÷\mܧ`W?í´5&Rz ¿¸º¦?Öjì¿å~SEÎ@¿å->â"Þo¿ïÈÇ.¥/¿ïýD™`AGNfsrq3FGL J0521.4-1740TXS 0519-176?ì͗̅³?¶Le™˜à?¹"GÁ›Òj?¶Le™˜à?êž8夵?ÂG}$v7?Ç͇im,?ÂG}$v7?íCyŠc#n?¢Q¬ê!:?µä3®ž²Š?¢Q¬ê!:?èp•â³q?¦9Zßë%?Î=¨u29Â?¦9Zßë%?ṨDy£ý?Èç²"ÉÐæ?܌¯w¸?Èç²"ÉÐæ?Ñsÿ›4?Í`màЇ9?çF8z2f?Í`màЇ9?⃹†Û<?¼»uÙÃL¾?ÚøŒòIçˆ?¼»uÙÃL¾?É{œ£º.å?¨µ×´Nª?é¡×tG?¨µ×´NªMIXED4FGL J0521.6+0103?ï2êÿÎèíÀ3Zº8u'SÀ:ŽbwÄ\¼À<]Ú{9@ IKèá«V?ÿÉÉã
?ÀSÒ:
²?–8…‹"f?Ùât¿D£ô@$3"¸¿ï㸌íº?ïÿº*2Ùq¿åò³{Âîý¿ßEœVã;¤¿Òê"ޥȿá1ªlÞAGNbll3FGL J0521.7+0103NVSS J052140+010257?ïÿ<Ðzp?é&w?|ÀìçÌæ?é&w?ï÷U²È?SÌ.ªöP?QTàãHNú?SÌ.ªöP?ï÷GKæTÖ?U͇•‡¨?Qqg£%y?U͇•‡¨?ïþL×I''?¸úié1 ?+2ŠnpºG?¸úié1 ?ïÿ&»ŠÚ?nŽ>)jQ?(£"yEØ?nŽ>)jQ?ï߬+¨¶~?|h"Ãeø²?p)ê:Í?|h"Ãeø²?ïøå¬Â–?XMl6`?OÜhèZ±1?XMl6`?ïú;1H)?@"n>æJá?G:‰–6]?@"n>æJáAGN4FGL J0521.7+2112?Æw÷cçÀ!iÓpóˆÀ6Þ¯\y}šÀ:­ò<ÈÞ+@]"ÿ‰b•?ýžøé‹Iu?'œÅ+	?§v™[ӇÉ@Çxþï^È@ȅ%ï'쿍4ö`€/¿ÙÇCáVF´¿ßûÛÙ>¿Û[$^.3š¿áø"ÁEZ'¿ÙÈý4s¥AGNbll3FGL J0521.7+2113TXS 0518+211?ï÷	RÓÑ=?] «bðW?QíZsÚfj?] «bðW?ïò—shqG?`¹èEææ?ZѵΠ'?`¹èEææ?ïjgêlgT?ïP`ÕV?'³·š€?ïP`ÕV?ïÿW÷7Úb?
™7"µç?pcç?
™7"µç?ïûÝ«@ ?@WÌý²û?@‰T«g)?@WÌý²û?ïµ
]sp?Œ±Ù"Kõù?'½h"­Ào?Œ±Ù"Kõù?ïÎí}¾¿?…ƒS+«?x‰A
¢øh?…ƒS+«?ïÿL6'8?ˆå~ÀžJ?|¡tBò?ˆå~ÀžJAGN4FGL J0521.8-3848¿Äq߉=À@®1¤½º
À9ò÷Ãñ[øÀ<Yñ›@T¹³?ˆ@"C'OH=?·1NA+™a?©v(ù!?íºôB\›â@'̳¢Y\¿]kW´>W÷¿åÔ"°Õ¿ê1"ÝIó¿ä\¢b•÷N¿ätSŸx"¿ïü¿øÓçAGNbcu3FGL J0521.9-3847PKS 0520-388?ïþõ±ûî¬?µâՁ'W? ¤áyX%0?µâՁ'W?ï÷ôn|­?RýXÆÄß?PÁ»y»?RýXÆÄß?ïðP"0èÅ?^§E€Ê	3?_^× î&)?^§E€Ê	3?ïÿ«Aãä>õ< ¯$"?/·Ôߝ>õ< ¯$"?ïÿN&å®?Ç,6NoÂ?v;´lìþ?Ç,6NoÂ?ïÝØ®b?|'|"êé?qô3°	?|'|"êé?ïè Àœ?m'´<n®?gßú­"?m'´<n®?ïÿ#ý5J?´°Kï×?[\Ò˜?´°Kï×AGN4FGL J0522.9-3628¿Ò›í±É¼À@\] l‡À7Ÿmži3À;¦¾Ë'Iò@ðáºÅŽ@øÛÎÈO?"¸ý?¹Üä?³v¸îôiõ@ôAÿ~Ñ@U9˜R¿Ñèb8Yc¿â|Ê@€x¶¿ç°c	º"å¿çJ0i¿çäGbj-p¿át>KëAGNAGN3FGL J0522.9-3628PKS 0521-36?ïý¥Øʺ?+àk¶…ô¡?2Ñ;PbXR?+àk¶…ô¡?ï÷&™‹›™?UëVµZY?Q²Í@¾Í¸?UëVµZY?ïךJyá?y'Ы«s?t2ÚèUSÃ?y'Ы«s?ïÿêþL]?…B'4ñ?'£3¶ùQ?…B'4ñ?ïÿQgâÎ}?›•‰$E?Ó/ÇÉ?›•‰$E?ïÚÆ~ÃÄ)?uDZ×uÊî?rœÀ¹šË0?uDZ×uÊî?ïØÁò "U?~E]~;?sŸ¨×_?~E]~;?ïýØØk2ö?*Üæ/͂â?19;Ôf•k?*Üæ/͂âAGN4FGL J0524.5+2839¿ÍÂ+Lùœ¨À*Éòý¸þÀ9€ŽÌܽÀ;âF¼|ó@ X#8lÄ?þV>¶4ž?»àçáÑ?º ïZP?ÿ¨Ec·_}@ {KÆÓ?ì½q +Y¿â¾È'«hÏ¿ÛþcEÿڕVß	æ3¿ä;uÂ#ü_¿ØåÑëð~ƒAGNbcu3FGL J0524.4+2839NVSS J052429+283918?ïúѹ+ìS?8Chr£½?D¹?+	?8Chr£½?ïÞÇ¢&Â?sbžR2t>?pœ.á 1¤?sbžR2t>?ïäے@œ?o¬>C<?k$m|–Ì?o¬>C<?ïmv=Â?tOŽg,P?'Q<ï°¸«?tOŽg,P?ïélX)?^DÈA¡F?f~"zæç?^DÈA¡F?ï&ÇÙ.@@?«Í(]u²?›'ÖÈ[ö?«Í(]u²?ï$yà ¸?ŒÀü7ˆ'b?ˆ¶á–
?ŒÀü7ˆ'b?íÅJ[‡©ò?•]\Ī~?±Õ­$0£ñ?•]\Ī~AGN4FGL J0524.6-2819?à›þNáÑÀ>c…@FA-À;"ƒ°jÀ<Ÿ˜!ÊU#@ˆâÖyt@®ˆ#Oa?ÛmN·ó÷´?̳ɛ"ñi?ðPêÄ.™@
'S6³ÆA?íJa¸¼-¿è3hb?_¿à5B!b¦=¿ë•›¨g'¶¿ïüËÝäw8?ïÈm54?AGNbcuPMN J0524-2818?ïô»: ‡A?}!"·¯'?V‰Šêì}Û?}!"·¯'?ïøÉ~ÊÇ?QˆSƒ-D"?OèÚRXތ?QˆSƒ-D"?ïv¢>ïô?Šó}x—:?'+¸?¢r?Šó}x—:?ïþÄ`dB?ÕNCö¿?#¹÷RÛùY?ÕNCö¿?ïýO%yƒœ?=Œ¬ásòœ?5†Òoüé?=Œ¬ásòœ?ïßÁ?/Á?qŠ†Üž–?p?BÛ{Í?qŠ†Üž–?ï_À¦?Ÿ˜³«î¥?"üÚ£Ón?Ÿ˜³«î¥?ïû"l€J­?7â€v³•?CvMø<r×?7â€v³•AGN4FGL J0525.4-4600?éjT.wÙùÀ@Öb=ú	À:bøwu'cÀ<dà?p@Ðÿ£ä¡*@'÷
èöÏ?Ãþuf^ƒÄ?©‰¼VÝÝ?ႣžU@#?ÿ·.Lïqè¿á÷ÀBû¨¿è¯•ÿÜſ㲁œøŸ¿à¡?«;®¿êp$ sRˆ¿åÛÍátϋAGNfsrq3FGL J0525.3-4558PKS 0524-460?ïñ™'ÈqÉ?`ôcFMЙ?\ÌúŠ™MN?`ôcFMЙ?ïóm@RÞþ?\?/Áá"?Y%~ӑU\?\?/Áá"?ïÒpÉu?t©zÇKK?vǛ[wâE?t©zÇKK?ïçŒB\àš?QϨlÿ1?hs½æw½*?QϨlÿ1?ïǹL½Gõ?yn;_c%1?|#Y¢»Ý¸?yn;_c%1?ïÎú'Tž?Wïõù?x'¾Ó9I_?Wïõù?ï£A¡òê?Škyªù®Ñ?‡/—|›Íu?Škyªù®Ñ?ïnѺpú?€ÞåÜóËf?'%ÈÃQ¹?€ÞåÜóËfAGN4FGL J0525.6-2008¿í¸ÌjÒ1À;ŒŸ±À:Ý
s†	šÀ<§Ç'#©R@ÚRý¨â¸?þÎE"I$?Î`ù•WÁ?ЬÞe%ž @vLe3`€@:@ºˆ'¿ïøªñ°²?ïöCže[O¿àdïY­¿ßÏËd—Ú'¿çf½+-«¿ïÿõEq#AGNbcu3FGL J0525.8-2014PMN J0525-2010?ïúf«Ì?8!Ÿˆ#m?FfØE-f?8!Ÿˆ#m?ïꡆÍäû?g@•}~ý?e^ym4Lí?g@•}~ý?ïŞTê= ?r€P/µÕ°?}0ՙÿ·Ý?r€P/µÕ°?ïÀtám1 ?a¾ÄÚ

?ŏ`›£?a¾ÄÚ

?ïòNò+
?Rù·RCo?[b…AõÐ?Rù·RCo?ï§2ÂR¨ø?(PI»Ø?†3Ou¤•ù?(PI»Ø?ï)wœA?"wjPÈó¹?šÑ®/ªr?"wjPÈó¹?î͓"=?f¥Y?£&ƺÐP.?f¥YAGN4FGL J0525.6-6013?Þµð»-À@ïz€Ïž8À9ۍs©ÏÀ<I<4c´Û@ £‹7?ûìUÿø?³Ãê%"N_?¥x¥X>°j?óo Ä0@?oߋì2?î*æþ§:l¿ä2ì@Ûgo¿ÞT"f¬‡¿ÐÍzÝð,¿â•†¢Z2¿¬éÏ£'7AGNbcu3FGL J0525.6-6013SUMSS J052542-601341?ïýI§Ø?,'Gq	‰?7]´R&î?,'Gq	‰?ïõ͓‹,?W< GpEz?TdÙú)ø²?W< GpEz?ïð()eà?gTõÚõõß?_¯­>&€A?gTõÚõõß?ïëa÷'$˜?M­Ì©ˆ¤-?džÓ\¼?M­Ì©ˆ¤-?ïùrñâ?EÐú—?Kž3'ÞË?EÐú—?ïÝõªL5?sЦg²'¡?q*Ðýͺ?sЦg²'¡?ïógäçï?ié¶7Ì?Y08_ '?ié¶7Ì?ïÈä›~(Ø?gïm$±?{²4ŒûÚ?gïm$±AGN4FGL J0525.8-0052¿ê'ÛÖ;F¹À3\‡D,»À9÷Í-DÜ©À<(Y‰QÞ@ÇRŠ¼\@C«Ë]a?À'Xßj3P?Ç¢C÷¦•+@܈皮m@
¯Ò"¢k?ïn¶—b&¿á×]Ÿmn¿ßr5§º¿ßO{hV+¿åýJä)िïñ£µ}AGNbllPMN J0525-0051?ïökÊ('«?P¤ÑÕy€?S(kg'Ê8?P¤ÑÕy€?ïóãïÿü?V—äSúBš?X8ñç?V—äSúBš?ïÚÿÖm0?uts+³ˆ?r€À‡ì1?uts+³ˆ?ïÓw£ûrR?TßFï?vD-ðhßC?TßFï?ïð©=j^?\iîGO+®?_Ê­®f"»?\iîGO+®?ïÒ`Ght^?~§Mzqâ!?vÏÜT´Í$?~§Mzqâ!?ï;ÉÑo?"çь¯cK?˜†ÅÞDd ?"çь¯cK?ïMuØZ†?{A°çÐq?–LQF¬}E?{A°çÐqAGN4FGL J0526.1+6318¿áÖæèƗB@.bTæâ!ÉÀ;"®"i›À=u‰ïØk@½"ªú¿ú?þ@ÊËjÍ?Ò¼)œ0¢µ?àÔ}e†l–@
dëVûX@q리§"¿ïÀ	ÿ÷?ïúDÕ&§¿Ì¹¯ä‰¬ç¿Ül±n¢u
¿ïÿ«±Ê?ïön¼v=tAGNbcu3FGL J0526.6+6321GB6 J0526+6317?ïì½cß^±?q¸Úõ(~?cBœO[þÉ?q¸Úõ(~?ïØÇÂKêd?{74p/H?sœÌL]÷?{74p/H?î—ä~‰?š£*1Äؓ?¯FCoåm?š£*1Äؓ?ﲍY^/?oãÏ=+?ƒyܨøˆC?oãÏ=+?ï¥õA­kÖ?'HÍó?1¬?†'¯ÅҒ?'HÍó?1¬?Èm—ˆ?² 1@óBá?§TCtÛ"?² 1@óBá?ëIb¤åÓ?±™òØ­´6?ÂÚulh³ô?±™òØ­´6?î'x5à{o?žÌü äŒh?­ˆ|¬Æ?žÌü äŒhAGN4FGL J0526.2-4830¿ëk`Ô´«À@à‰~™cÀ8QÔâEÀ;Œ½vîsç@ðmBùyÔ@Ï7ûïÐ? ¢òˆÉ×?±)¸
Hx@¾å@a @a v­†?°`Úá7'é¿àúõŸSí¾¿äv^½|¿ã–Ð[͆0¿ç»ÙÊâ¿ç^1¾éà.AGNfsrq3FGL J0526.2-4829PKS 0524-485?ïý¤G¿ÔŽ?&'_ül¿?2ÝÀWؽ¦?&'_ül¿?ï÷*Z‹U£?TØøPA?Q«K%ÍÙå?TØøPA?ïãNa6ý?tT+†¯œ¼?lí±»¥»B?tT+†¯œ¼?ïÿ®M¨ è>ôÉ3N
?l˜ÊÏÞ>ôÉ3N
?ïþ;ã8§š?#VxÖÖH?,AÏíî)L?#VxÖÖH?ïáÔ+™i|?o}¸*¾ñs?n+Ôq•DN?o}¸*¾ñs?ïèX´Õ'Í?t#†NWŒ?g§JïSë©?t#†NWŒ?ïÿk'Quá?	æØr{6 ?¸"ôü?	æØr{6 AGN4FGL J0526.3+2246?éJb…oÀÓÅyò4eÀ:bnŠ!WÀ<–C£Ã¿@!›i}r?ÿœ
Ý©"ã?Æ3–ÛNDÜ?°,¡r´?æ"ÿ[•R@$=Pš¿í®,Ε#é¿ì÷iCy¿ÔDhz<Ý¿à- Qn޿嚌Wè¿ÂèL:wJAGNbcu3FGL J0526.4+2247NVSS J052622+224801?ïþúýÙÓ?™QI"? P-2žÓâ?™QI"?ïòz'RC3?dy³
·ù?[±n·j¨?dy³
·ù?ïùÈÝK^?A1íEн?H܋éN)?A1íEн?ïû‹†ÜR§?0cÍ¡€ˆg?AÑä~7E?0cÍ¡€ˆg?ïÿ³Ëžú?õûÑ×?)‡ÈɀB?õûÑ×?ïÇ@¼'Hñ?…²όj"?|_¡Ôè+x?…²όj"?ïøSsrÐ?bvG`ó—?N³æ‰žt?bvG`ó—?ïí7Jð?XÌ¢´L-?bÈóFŠ?XÌ¢´L-AGN4FGL J0526.7-1519¿àâZ‡NØÀ9~ÓØYÈÉÀ:d)uDÀ<FøE ›@Ý7•B?ýçOšr®?¾öڒ]:?ÁiíˆQ@ÅlC9@֌W¼ªk?ïÿÐ/WÜ`?Ö~?¶N[¿Øò°¡ôó¿àkÑtÒ9ô¿èŸÑâ5iÄ¿ÇE"/_iAGNbcuNVSS J052645-151900?ïò'G .?aù¡`CŽ?Zàû‰U+?aù¡`CŽ?ïÞZ¥py?p"±²tnØ?pÒø¬—×±?p"±²tnØ?ï"
<LÑ?ˆ"ªDØ9L?Šý|&÷Ã?ˆ"ªDØ9L?ïJfß?~`–N{°?œÜ–­ü´
?~`–N{°?î­GÎm-L?¦¶¹­8Ç?¥+ƒ™v>?¦¶¹­8Ç?ïyp\'Ø?'±só¼?Ñôow2ò?'±só¼?ìâŒ$*›?ªöò¼ÕÆ·?¸ëžàZ'+?ªöò¼ÕÆ·?ìuÄCÖx?¢*e6!?¼QÝáOÄA?¢*e6!AGN4FGL J0527.3-6223?°ɟéiÀ@ÀœÜD9À;ÝùzªÁ	À<ý'œüûi@!ûÛ® ?ýç"Ä!?еâlvK?uÁ	þB?°ÌáßGgŒ?òBxåÄë¿ïþ×áÓÅ?ïÿJbú¡¿æk´ÿ{ µ¿Ô…4‡Ç	>¿äŸùš‹1!¿®$æ¿<@xAGNbcuPMN J0527-6225?ïþbÈ|\?'ÁA7dn?)Ӄgü¨P?'ÁA7dn?ïêƒE^Û?r+Ô1¬ˆ§?e|º¶€ÍH?r+Ô1¬ˆ§?ïÔS²bEù?{b²?¼.?uÖ&Ó¬w†?{b²?¼.?ïè–ÑàT?SÇB™›{?gi.H»ü2?SÇB™›{?ïþP@ÆTõ?0…²ôîÜ?*ûðdAlV?0…²ôîÜ?聾‹£?h?˜oÏrxÖF?†žÀ‰ð?˜oÏrxÖF?ïÙ%2"|Ï?{'àëMM‰?smfÀlX?{'àëMM‰?ïYM-|²P?ˆNŽÙL7?"ÖZPi¶
?ˆNŽÙL7AGN4FGL J0528.7-5920¿á¶5ü¼(»À@ĝàP7PÀ:~Æ/#ÚÀ<¢Û2Ál@|1~Ó?ÿþí+%Â?¿€®¼šq?­rp#ÃBy?ñ¨—³æKú@…žß(Äð¿êº ¸\R¿Á+m—C¿äOc 8o2¿Û¢"#揿×è÷»7ùì¿ëëgÝ^ëHAGNbll3FGL J0529.2-59171RXS J052846.9-592000?ïþ9ÊY³ƒ? ŠiyÔcP?,cVÜû^Þ? ŠiyÔcP?ïöð~Ð?SŒÍùà«?Reg8K?SŒÍùà«?ïö",®oü?\™s½¿¤'?Rצ°Þxª?\™s½¿¤'?ïü‡KÓ?"­öaؚ©?;Å¢oÙ½-?"­öaؚ©?ïý
­?0n[ú§ˆ?7¨ŠM£XT?0n[ú§ˆ?ïÙÅi^Æè?~í#MǼø?sKL}Ó?~í#MǼø?ïö<?ÔßÉ?f³7bµ\d?S‡èLíà?f³7bµ\d?ïò–«'¶}?M¿' 	+$?ZÒ©[\µÌ?M¿' 	+$AGN4FGL J0529.1-0101¿ïût{/©ÄÀ2¸Å¸ÜUÀ:'ËÌòŒzÀ<#WóÝ@åü¤«Æm@'Èš8%
?Ýhüopü?Û*à~Zxò@0…ÔÀ·?ù|*­þ€y¿Ýpõ³ ?ïzËx8ö¿ç§¬_nû¿ë+$Á€hp¿Âðvà‡Û¿ï|þyØAGNbcuPMN J0529-0058?ï)Ô°y"?¹ËŠS;Ír?šÅiðÎMš?¹ËŠS;Ír?î.¿aº°?³
y8›¿ô?­(,‡?³
y8›¿ô?î:˜8µB?—ºÀ5Îä?¬V|vc­¦?—ºÀ5Îä?î"Mp(å…?—A+Ú©xB?­Û(û¹Ù²?—A+Ú©xB?îM#É«'?³:EIîÞ?«.-Á­˜?³:EIîÞ?âƨuKþÓ?Ҙ-Pù H?Úr¯hY?Ҙ-Pù H?é@ê(ä?¶Èì
´èb?Êÿ³°W\n?¶Èì
´èb?Ù°ºEê#?Ãý[2ß.?ã'¹"Ý
ï?Ãý[2ß.MIXED4FGL J0529.1+0935?ïYÎìØÀ*Ú ¼8*À:&ä›ök,À<[}Ë@ C~Öʧ"@†‹ýϤ?¼x‹×åп…aC^EýÞ?Ëxëä•{@gmrU?á5žÎ^¿Ú>(¤äÑP¿èQxbè,¥¿á8Ï>ìúÀ¿Î/~Ȳ῿áå]‡š"•AGNbcu3FGL J0529.1+0933GB6 J0529+0934?ïüÎY¿g?)˜Ў¦?98¶‡"?)˜Ў¦?ïõ_:x ù?V¸p×Q?UAŠ½Gn‹?V¸p×Q?ïø-WH‰?>þ–&æº?OÏIØ»I?>þ–&æº?ïû	ÛÎr?*l]áðŸ?C۔°?É?*l]áðŸ?ïü5yÎ;ü?2/˜`XŸ?>T1Íå¨Ò?2/˜`XŸ?ïÕÞ¢sn?| 6ÌåH?u®àeù_?| 6ÌåH?ïîÄèÁŽÅ?o9_ÜWY?a;v;O?o9_ÜWY?ïì*a8»D?SxêÌü?c՞Žë$°?SxêÌüAGN4FGL J0529.3-7243?Þ'XúºhÀ?à.D¶é6À:YDéN
À<Q+"€ä@mÑ Ç
k@™µc#»Ç?À*ZÜð[r?±:ÂÇ;=?ñ4+
oÆ@4"Y8«m?ÛL»ð[¿×cL@Í¿èd^y]¿Ý"Âãü¿è˧¾uq¿äm´8PÍAGNbcu3FGL J0529.8-7242PKS 0530-727?ïüÿ½îk6?6vüx'¥?8˜i?6vüx'¥?ï÷a&q¿ò?Vª³x5r?Q=³Mú{³?Vª³x5r?ïæwWÇ´?qk7²Òe?iˆ¨Z§–\?qk7²Òe?ïþÆîLµw?
_æCÓ'?#'²ê‹å?
_æCÓ'?ïúÿ{±ãN?B¸"j?hš?D'›¼?B¸"j?hš?ïÙjZî?€Ï^iÆ+ï?ssÊÒG:?€Ï^iÆ+ï?ïÔ³Çí9?€aó+°ƒÓ?u¦p¹O'?€aó+°ƒÓ?ïü\#ŽÇÑ?/–ÒEÛÍ?=ãÊ -?/–ÒEÛÍAGN4FGL J0529.4-0521?âÀ;vp5À4§"BAÃðÀ:	"V!uÀ;Údµ—&@'»Ÿ}ß)@E&z¾@?Èi
!A?Ñøá}³à@)=Ùb·@´Ž®¯?ÈqȨü¿ä®Á~ºñ¿ço£üÉë¿ë#3 hÖ-¿åù)Í¿ïîäŸQiAGNfsrqPMN J0529-0519?ïàyo'™Î? jAmVÇA?o†"c²? jAmVÇA?ïÆéh¹ÒÊ?}^•ñF9W?|‹K£Æ†ö?}^•ñF9W?ï‰^véýp?"@!©4¯?¨b;1Ïô?"@!©4¯?ïBceç!?usŠ­ÂÂD?—½Ó"úéå?usŠ­ÂÂD?ï̸•æº<?xÞÄã˟?y£µ,?I§?xÞÄã˟?íì^éM¸?¶(r)DW?°´M‡Å?¶(r)DW?ë¸Lp#²?«ä-²,òÙ?ÁÎ?q7®?«ä-²,òÙ?çSC"—²l?³|÷$ù¯?ÑYxöЛ'?³|÷$ù¯AGN4FGL J0530.9+1332¿îÊ`UL°À&YWŠ*'À8Œ×òš½À;={á!îg@%C"d(I@­
?#?­êYXR…?ÑÅ9$ä»×@¤
COàé@0à?ÊN½þ'㟿Ûé
_¹ùá¿èVݲME¿é55¬E¿íàpÀ¿Ý,_#ÑìFAGNFSRQ3FGL J0530.8+1330PKS 0528+134?îüög>ÂL?­Œ0ún§›? 0™ŒïÂ9?­Œ0ún§›?ïÚ"aeú?y Üڐ¬?rîÏ8ßZô?y Üڐ¬?çiɨˆ¨c?±èÐô?Ñ,l®î¯:?±èÐô?ïáÙÿC…?_8«ƒÙY?n&˜÷Ë8?_8«ƒÙY?ë»›%hx?¸ÚT?Ši?Á©"j^ ?¸ÚT?Ši?ïi|Îæ5?°†3ûÎû£?Ÿ²Ð]Œ3f?°†3ûÎû£?æàSž§dL?²_àÖ¾?Ò?X±7g?²_àÖ¾?î`¢e¬=q?˜¾|DLŸ¼?©õ١̌ï?˜¾|DLŸ¼AGN4FGL J0532.0-4827¿ë)H3~XÀ@fýüÁrÀ8;u!MÀ;g¤(hÔÖ@]
È°ÞZ@±ƒ›*"R?žTþ£Î?­?³è'¦
k>@c5X§a@ 
2~,€¼¿Ðëæ£7¨
¿Û@.Ä8©•¿âËcÁ'ý¿â[Kµà÷ý¿å6±'n"ÿê^òԞAGNBLL3FGL J0532.0-4827PMN J0531-4827?ïõeCÿy?…6—¼€ÁŠ?U5yX?…6—¼€ÁŠ?ïöåFº=?S¶&Ù
Û??R5ï…ÉU?S¶&Ù
Û??ïâ"Ç{2?t˜×/ÜÑz?málr>=Ø?t˜×/ÜÑz?ïÿñ[É´>×&€ƒAf>ÝIþ3y]±>×&€ƒAf?ïüºg^LÖ?1€ÁÌ:??:,Æá3@?1€ÁÌ:??ïÚÏè=Ê?t¾(Û§…?r˜Ç"?t¾(Û§…?ïÕ?*?ø?€ý=BT³?u`jø6C?€ý=BT³?ïÿë"a½Ï>ßêk8ihq>ä{‰ªÞv'>ßêk8ihqAGN4FGL J0532.6+0732¿ÞQ_½À+uîÇÉXÀ7"ñÓ'éÀ;B™Øƒº4@äÄ*;è¹@ž{€©ß?—w¾8Ɓ??¸
Xs‰@-š
^ÿ@kß/ûÆ5¿Âç<9¿áyÛX€Ê–¿åô>‹$¿äN'ÿú ÿéÂ}h‹…¿í*7/AGNFSRQ3FGL J0532.7+0732OG 050?ï÷Ðæ%Ó?O}¥# ?P^4&lã?O}¥# ?ïá ³B¦Ý?uîaûÓ4˜?nßLæ"r^?uîaûÓ4˜?ïÞ-ù2Ë?q'-lz÷ ?péÅ2"?q'-lz÷ ?ïñt=ƒ]?NÞ¯-6àƒ?]"º
$O?NÞ¯-6àƒ?ïìsÏ8?•?bÚ$ºÑ¢÷?cŒ0¬C‹?bÚ$ºÑ¢÷?ï{'X:\P?¢ÛLu<?´ó
?¢ÛLu<?ïÏÞMtè?蓁™t
?xـ<4?蓁™t
?ï çË?y+î4£?‡ÆAêAc?y+î4£AGN4FGL J0532.8-3941?îî4/ÝÀ?p‡¨ÖMÀ9¦Àð¸,À<]sWN›@¯B¼I@hÀ³¹Ö?°°"Üj ?¢ÊîË	K?ì•Õ>á<F@
£	Õk׿¿ß^TùM¿äÀVìÔª¿è¡Ü>ñ§¿èáyaë­c¿ßúþÄÄ
¿æïËoÌÂAGNbcu3FGL J0533.0-3939PKS 0531-397?ïÿ=Þe"?	È7'žc?D1Ly¢Â?	È7'žc?ïø%Ò2Îp?P5+ ¦a?Oh·)ǁŽ?P5+ ¦a?ïññJ–¸O?cx¡Š0?\jIÐ?cx¡Š0?ïþ½—?;. £Å?$&'°6Œ;?;. £Å?ïÿ-÷T?̀ü*p?VzD's?̀ü*p?ï݃XºF?sãìqØ]?q>S¨î©?sãìqØ]?ïìáå/;¤?kÁ_CLÿå?c¤É\?kÁ_CLÿå?ïúÒ7éY?<D
á¦?D·ºEZ	?<D
á¦AGN4FGL J0532.9-8325?ë"oIu%,À='xÝao‡À:ž‹¦'Ï¡À<Z›•\W@ ceù"ð@$á{°z‡?ĨèÁõÙ6?½š¸}ŠoZ?øNbS—@·ww°»Ÿ¿Ù‰§^(T]¿çv•žoû¿äêÖù¿ß ¾Q	¿ã~ÛþZ¿âÿ90£6AGNfsrq3FGL J0533.6-8323PKS 0541-834?ïÿuÖhNj?±WB§]ÿ?E6±t(Ÿ?±WB§]ÿ?ïö$- "?V"ïÆÕ?S·¦4³—?V"ïÆÕ?ïúÏIÝLT?Sx JÕ?DÂ×~†É:?Sx JÕ?ïÿ£[º:ú>ô˝+Ц ?)'³T1>ô˝+Ц ?ïÿ¹|ÊB>ú-Ò·šˆ? Ê¡œ''>ú-Ò·šˆ?ïÜ6Z7·…?}Òh«¯­—?qäÒñâ­u?}Òh«¯­—?ïüSì¢fX?RÁ,f­Œ?=`šqYË?RÁ,f­Œ?ïþÚܸ…Ì?Ždó«Î?"R6³bCõ?Ždó«ÎAGN4FGL J0533.0-8446¿Û'Ð+ځõÀ<Ädf±åÁÀ;g
ÑZÀ<…ÚcŽDÒ@ùX¾2*J@œÈ='?É<;±î?­Ø°A ?Þb§Êà@ÅÌ8þ#\¿ÊEŸœh?À÷ö†¯‡¿ã{Âîýy=¿ègÍ<^¿ÒÞI¡ßŽE¿ïõ£ñpwAGNbcuPMN J0532-8447?ïÿRðV®|?ä]Ùÿ>?¡û<Úá?ä]Ùÿ>?ïõ}®_,?[ò͝Æ9·?U£Ày8?[ò͝Æ9·?ïñ±Æê":?Vâ#"³q¡?\œr¬
ۉ?Vâ#"³q¡?ïÿ"ÀU‰ä>ù<fž¶?êÇ¿¡l>ù<fž¶?ïÿ&ï-ò?1O¡ð?""tçq?1O¡ð?ïÝ­¾¥ÓË?~'ý{a?q) ¿£þ|?~'ý{a?ïñkriÔÛ?fp«DÙý!?])hÏiæ?fp«DÙý!?ïþ~ë9ì­?!yOSä6
?(J0tïÆ?!yOSä6
AGN4FGL J0533.1-6119?ï†<%†]ŽÀ@s(bõ˜žÀ:¨`"†ÉÀ<bûáN2@õÉe²@à´Zåÿ¤?Ì&ñ[wu?Çö?¨·o?ó	7KƧð?ïücÍÒ'Í¿ÕÙ6ýîü¿êBjۖ"¿ìÂ¥â'Qþ¿æ_Ë‹«D¿ïúè3Z `¿çb¿è¸¼AGNbcuMRC 0534-613A?ï‹l3bŒ?³ˆÃ0toœ?>dú•?³ˆÃ0toœ?îµ,x'?ºr™iaÝ/?¯t­<hÚî?ºr™iaÝ/?îf½'p€F?šlè[ŸÌ?©"&éÓâ£?šlè[ŸÌ?4Ì%?'詵3<?¤•ì´öK´?'詵3<?ïÅOåña?Šg…–|?}Xð¢º?Šg…–|?â È
0¦L?Ó`Xôý‡?Ú¾o垳g?Ó`Xôý‡?íd&ª' ?¤ƒ£™9ÜÌ?´Þʯ0ò¡?¤ƒ£™9ÜÌ?ÞÿIsˆÛ(?Ä®,û®*?à€[F;'l?Ä®,û®*MIXED4FGL J0533.3-5549?ïÛzBÍk>À@}Š2ôIÀ:')óÀ<rfàß©H@ý܌ˆd@£!ØG?вLBù¤Ç?ÕRåB˜?ÿ0ÈÚÏÄÏ@rßÆ?é¼|±¯¿æ_(뱔¿è'm{-ž¿ìâô÷ŽAw¿æ©Q2!»<¿ïÿ°NçÄ AGNbcuPMN J0533-5549?ïõ@¹®Œñ?N·¼sjt›?U~Œi,®Ó?N·¼sjt›?ïã²I
Wi?u[—µ5?lM¶òèæÄ?u[—µ5?ïg !Õà?ˆ5Å5‰È?"ûÍÛ‹?ˆ5Å5‰È?ᆱ¿ênÒ?cæ€ÛND?€Uù³ž?cæ€ÛND?ïò¼ÌŠÃÏ?^õôLdOê?Z†g`ªñK?^õôLdOê?ïi h?š)Ƒ¹M?'ÍûúK…ñ?š)Ƒ¹M?í€SNŒ|?¦ížP#7?³ýe»j?¦ížP#7?헥:Y±?¼´er¬?³BÖ.ïXr?¼´er¬AGN4FGL J0533.3+4823?×Vršs«–@ {z_A®÷À8t7	‰À;ˆ"/•ð@ï-Ì­B@–n^'lV?T뱤í?¶./g5Ä@øDIÛì@Ðw€üj¿¢ÞAbd¾¿á›CRe'¢¿åÉ(½äQ¤¿å¿˜f"²Ð¿è§ÂòXw¿ëô—ìñ/ƒAGNfsrq3FGL J0533.2+4822TXS 0529+483?ïøŠ€Õ†?HδUcvn?MÕý¶÷(?HδUcvn?ïØu8!•¸?†Æ!"i«M?sÅcÙ7¤?†Æ!"i«M?ïßpÓÒ¥?pž—ˆ±å¢?pG–Ý̜?pž—ˆ±å¢?ïïò}zC?I`<¤0ù?`
'TBŸO?I`<¤0ù?ïö»í›=M?OÁcw,C©?Rˆ%)ºvy?OÁcw,C©?î¼BÆ£g?µ6fSe¡?¤;Ӛ
Fš?µ6fSe¡?ïÙÑùá?Î.I³?sx—Z•óÖ?Î.I³?ï²âúÐZ?rç<	ÿ†Ö?ƒGARÈ´@?rç<	ÿ†ÖAGN4FGL J0533.8-3749¿æo¾*üÀ>ÜÊ>}QÀ:¬6ÉÀ¨ÒÀ<šq
"=@ba§ºÄ@m(<_+à?ÅôšÇ)?ÃCOàèã"?çÐ*_z@ ›'
`?ïôb¦h_¿èuüÜ_¿ßéÔ¯ð4¿ëƒB‹?å¿åÇ-†K<¿'üyº´¥AGNfsrq3FGL J0533.8-3754PKS 0532-378?èïÿÔqÝ?ÙòèV!}?Ì@®8?ÙòèV!}?ïøqo¦M?R'¿°žL?OÒ9á¾wX?R'¿°žL?ﯛYôNW?‹ò;Oò?")ˆkÊ+?‹ò;Oò?ïý¶0 ~2?úu¶•?2N{v+"?úu¶•?ïúþpUJ?L÷…KU8ß?D?nŽˆ‹?L÷…KU8ß?ïßH>LÕ?q"U|@?p[àúIéH?q"U|@?ïbêë)?"2zì!?"¢¿e¹ Ô?"2zì!?ïø§•
o?=ÿ&iÇc¥?Ma««£n®?=ÿ&iÇc¥AGN4FGL J0536.0-2754?é£îCøÈÀ;ÝCá`xÀ:ß9á£À<]HœQÿ@·FŽ"½"@Õ¶€Z-?Ëîc cbP?©sŠd§?ÖÏþ…Š@–ˆ¼|ž?î10Ÿ//ÿ箅^¤%9¿æÓZ»7y¿å·Š`@²x¿â¼(Fp'¿ïÿËA²Q÷AGNbcu3FGL J0535.6-2749PMN J0535-2751?ïþˆµàeö?!U¸ý5Âÿ?'tž[Ö¸a?!U¸ý5Âÿ?ïõê¡ã®Õ?T*X "??T*»óê%¬?T*X "??ïðÚ±øò+?]%¤5Ù±?^Jœ:©ö?]%¤5Ù±?ïûtKg˜§?%ҋ5¯r?B.ҕJ·ý?%ҋ5¯r?ïÿAŽ0Á?ŋѡ@å?ßÆpEsV?ŋѡ@å?ïØLœ)°—?ƒdê~Ñ#Ä?sÙ±ð§P?ƒdê~Ñ#Ä?ïæ·'&¾
?pG&ýƒ|?iHØ«çÊ?pG&ýƒ|?ïæcjnÄë?Y&òëÁðÖ?iœ•©øDö?Y&òëÁðÖAGN4FGL J0536.2+1733?ïÞ´D&ßÀ5çB™Ø"À:Fêóÿ@½À<eO1Ì@}4‰¢?þFÙóü¼?¢4GÛ5ñ?Οÿº4ï¡@ÃÔ»®—X@Jæº3Âû¿ïþR`Ÿýâ?ïýýu‹r¿ÏëŽÄS‡¿á9‹Â@Ð¿ä,õÌ W#¿ëþ? ÿ¿hAGNbllTXS 0533+175?ïé'Ùi›Ù?d•Þ×Aìô?fm&ugç—?d•Þ×Aìô?ïί–í(?†
øˊ*Ü?x¨4˜Š9M?†
øˊ*Ü?ïŗ(G"6?|× ±Ó?}4kâe1%?|× ±Ó?ï–Åg©ï?h+g†ÿw?ŠN¾ØWp?h+g†ÿw?ïŸ7•=?‡Îÿ¢¥€?ˆ2÷{xÒ?‡Îÿ¢¥€?îбˆÎ›.?¬U=?
¢?¢ôçr:f ?¬U=?
¢?íxü±tŠI?¤+šCªÓ?´8sƸ?¤+šCªÓ?íÌy'Íé?™Ï½Ë…­‡?±ŸT7/"7?™Ï½Ë…­‡AGN4FGL J0536.4-3401?ïL›G!ZKÀ=}Š2ôIÀ8¡è
šó6À;Ý6'Ú9@©½H@û0<Þ­ ?¦'a;Ú È?µ'ƒ§"Ùì@í'ÞkZÂ@/cê¶Ó¿Ø6µž²Þ¿âÏi)Eƒ¿éY£àDxÖ¿æÖ_îÉ¿ïCB	[¿ïÿ²vìAGNfsrqPKS 0534-340?ïúŠñÇ>T?;Û,œ¾?EÔ9çœBú?;Û,œ¾?ï÷dôæ
?Tˆø޷Ԙ?QË6t;e?Tˆø޷Ԙ?ﺶŒeöÌ?€/Š´/ç?R\àªöö?€/Š´/ç?ïÿ}¯`ÞÆ?ôÌej 1?J»}C?ôÌej 1?ïü|©ãƒ?5/Ü,¯N??œÌ`˅?5/Ü,¯N?ïà²_Ž0?qeÅFœ?oM t«ý?qeÅFœ?ï¡6ëñͅ?‡WÑò'Yž?‡²E
ÛrÈ?‡WÑò'Yž?ïþÔZFÕ?@Ö7'ò¼?"º^7í•P?@Ö7'ò¼AGN4FGL J0536.4-3343?ëŒüÀãèüÀ=h"ƒ‡ß]À9L&ÉÀ;ÏÏò=@!‡	^Ú+?ú|Y¸:m?´âlFOD·?»rØ Ñ­m@
pÇZ@©U¯	¿ÙZÿ**¿¿è֞b+CP¿Ñ'd@ò8—¿ÛúcWh¿×?d"cýV¿Ð"c:AGNbll1RXS J053629.4-334302?ïþúXÇ÷?֋+0? Zu0$[?֋+0?ïôý'n§?T;§ôlÎ?VúÕº'V?T;§ôlÎ?ïòzÔ»b?fUtp#ƒ?[
V?±¬š?fUtp#ƒ?ïéµv"?Q<	Ÿ?fæK*£%4?Q<	Ÿ?ïýE]'<0?,¤í|ô?5Õ']ôè?,¤í|ô?ï×m|Q¬'?u˜àeʍ?tIAºLþõ?u˜àeʍ?ï֞Ñ֐µ?'¡%•Âõ¶?t°—.$Á"?'¡%•Âõ¶?ëhÌÑ?z)kšÀÿ?ˆ…0ŸÅ?z)kšÀÿAGN4FGL J0536.5-2548¿îØi ˆ"À;Á?ÐÐhÀ:òÚ¬‰`fÀ<¦"Òb8@ 8»*
Ä?ûî[ãU¥N?Ç.DáÜS?Ãí†*Ñæ?üÉåvç½ê?üku.€F¿ìðdaS'?ïâèÍ´SY?É.Êî¦;i¿â5Z 	 =¿ÛrMºÈé=¿ÝïN¢$'–AGNbcuGALEXASC J053626.90-254747.9?ïþdŸðSm?!VîTo{ü?)¶úÞñ?!VîTo{ü?ïíâ|?fSu¢^Y;?bþŠÓûº?fSu¢^Y;?ïèkJ#á?idx/P¢r?g"µò|G?idx/P¢r?ïÈÁäD?`¿)üҖ?{ýŸÌñC?`¿)üҖ?ïõô±'*?O?"ÞR,ª?Tµ¸ÜE?O?"ÞR,ª?ï ÷AF?"u"}¸*?‡Â/̺k?"u"}¸*?ïÕ:#^Ì6?wŽúÒ?7®?ubîM*I7?wŽúÒ?7®?ï%wWi7@?†®)'ÿhú?›Q!J?†®)'ÿhúAGN4FGL J0537.7-5717¿µ½5þÈ%&À@2'!%¶À:/Pž~éÀ<}`Z³«@ñ:ǧ?ý~"_¦XÅ?ÁÁ¹my?ÆBº$Sœ_@w´_½Œ@j/š¢X/?ïÉ­}ÒÝ¿æÙäãD¿Õë&>®Ÿ¿ÜèÿI Û¿ãèZ&½+¿æDiò!vAGNbll3FGL J0537.4-57171RXS J053749.3-571844?ïú>Ö2.Ú?C7éBÜuÍ?G§T‡?C7éBÜuÍ?ïñ͜D]—?Ybϑxçá?\dLJÂòM?Ybϑxçá?ïíòùKÑ?d3½¤?b
£7?d3½¤?ïÇ!õs4*?^÷|Á?|oXóÎÒ?^÷|Á?ïîñ­VåÀ?VžOJèÉê?aR Û0)?VžOJèÉê?ïÂòéõ…0?†S{ÀѸ?~†‹Kë¿?†S{ÀѸ?&¶ÖŸ?¯!5òº¤?ŽSvGû"U?¯!5òº¤?ï'nÞñÇ?'׬ž‰æo?›$=ù•?'׬ž‰æoAGN4FGL J0538.2-3910?êN€e.ò¡À>LøŠ/À:îäŸQiÀ<­C³³÷@ ͪÃ7£?þS#ä
Öô?ÄUaÆÄu?±ÞfRDp?îªõÂ9uí@}
yæ ¿î˜×'2tÇ?ïömzVÞ3¿Ø70£‹àÉ¿Ý;êý9|#¿ã2½ÂmοÜl+Â{AGNbll3FGL J0538.4-3909NVSS J053810-390844?ïÿžõè¾µ>ý…G¾k
?BxóþY>ý…G¾k
?ï÷*&
?RÝëëN?QÕ¬<-³?RÝëëN?ïøgtKT?;A·Ö֛ð?Nb0—Î()?;A·Ö֛ð?ïþlÐôàÎ?f]ëºûˆ?)2ìxºü?f]ëºûˆ?ïÿ'ï*'?º¤p6ù­?D?æþKØ?º¤p6ù­?ïß*ÇÌ)[?qGVëDF?pjœ:ç'5?qGVëDF?ïùz€àÌD?_=7)H4?Jû°ÙS?_=7)H4?ïü9ç#Ýw?2ÿA 
Ó?>0ű.Y?2ÿA 
ÓAGN4FGL J0538.6+0443?âì^Ÿ¿ð¾À+³ý">5ÆÀ;]{ÜqÀ<g$€	@!Ã%	òó?ò«^Öw?âvÞñ'?ãÓÓÃt^@ÆQÒZ«@"6ÙÁ¿îè"1 ‹ü¿âݜ'éS¿ä5åàD"ð?â¼(+ì¿ØÖ'\ä¿àJÂ7óaAGNbcuNVSS J053847+044222?ïûÐbzëÑ?=a£óD)e?@¾v|ÄÛÁ?=a£óD)e?ïòNLÐNs?\ßDΰ	š?[cfž›ê2?\ßDΰ	š?ï«?½ôÜz?€­/w‹­–?…0µf?€­/w‹­–?ïöS¬$‹¦?B|•þ(åu?SX§þ`"}?B|•þ(åu?ïø—^q?Nd` lˌ?M¢‡Vk??Nd` lˌ?ïËMܵUÀ?…h~ßþ±?zYƒ¨ô?…h~ßþ±?旅XJÕø?‰X.»
tÑ?†_)âû­ù?‰X.»
tÑ?ïÚ­LB½"?pV)¸¤7?r©YÎ#H?pV)¸¤7AGN4FGL J0538.8-4405?Ԇ—N:˃À?"á¬WâÀ6…C>C1®À:áUÁÓt‡@¹&>{@%ن³U?…/‹]ìšH?¯¿!M@$qJG
@"_ða俚£xHCÄ.¿ÝUý£z´¿âŠ¨ÀSÓ¿ás¤r:¯ÿ¿å~bÁ–7å¿æHdÞ&‹AGNBLL3FGL J0538.8-4405PKS 0537-441?ïÁô=mãw?±uK±Sx?áQMTd?±uK±Sx?ïå¹viú×?®m8Ú~?jF‰gk?®m8Ú~?䀘z¬Õ?ŠPeÃà1\?…!_lÃ?ŠPeÃà1\?ïÿ™²\øÃ?	šl«¬í?	"x0îN?	šl«¬í?ïòSx¼Ä?UÀ㌠?[Y†öß?UÀ㌠?練HÆN?šoUÌú=?†ZmØÍ@x?šoUÌú=?ïÍõ˯/?…¿ìõ¢'?yy¨–ÄI?…¿ìõ¢'?ïþځsæŠ?!°ƒòñ]?"Wæ °¬g?!°ƒòñ]AGN4FGL J0539.0+1644?ÛZ­ÚˆÀ²ðZpŽÞÀ:?LÔÄèÓÀ<ƒræ§i@ À-+1\?üF€'q^è?ÇÄÚº÷f?Ð#nå;µ@`q$/Š1@Rëä?/@¿ïÿüñý?ïý~›;…¿ÜkÊSuÈÚ¿Å÷÷ÛÉ¿áL«tp–¿ìÓ51:4¯AGNbcu3FGL J0538.9+1646NVSS J053855+164612?ïüq¶â»Þ?3rÃ|'?<rGÒÚn
?3rÃ|'?ïì"Î;G?g^›ŠÃ9'?cÝ2ˆg?g^›ŠÃ9'?ïÓ(ªV3?vêÒÙÓ?vkª²–vÂ?vêÒÙÓ?ïßÐ1}Ý?RˆON¯«ù?pç`_?RˆON¯«ù?ïúº¤^Í?Aïb¬#0?Emû[*ž?Aïb¬#0?ï¨Á'ÁÕ?Mò@®r?…üO«À¶à?Mò@®r?ïW~¿M³<?'©æaÎ?•(fx?'©æaÎ?ïzi·˜vô?»Š5ʦ?²É¨ï‹?»Š5ʦAGN4FGL J0539.6+1432¿ïûôGm°À!_ôºQ À93Ô¶¦ÛÀ;©žÙt{@ó+kh®À@}/Bãª_?¹LFT£w?Ågù¹iï@§î%âè˜@çZ™B?ïø¬N¨À¿Ýã܉Ù2¿ç1Ubˆ
{¿æ'òÁS¿î™i}Èâ¿á€‡—ůAGNFSRQ3FGL J0539.8+1434TXS 0536+145?ïõ,Cš?R
˜M&îé?Tý§¾<B?R
˜M&îé?ïóEy~=•?[ýæ¿wÊ?Yu¶–d?[ýæ¿wÊ?ï™~7­/<?'%̦_óT?‰ r#Ìß?'%̦_óT?ïüGNH7|?*žïÞ?=ōÛóðñ?*žïÞ?ïãX¼–Ù?jçUÏc?l§D¿$?jçUÏc?ïÊì
‹‡?aà³Êv?z‰ùÐE?aà³Êv?íØ3«©3?£ÞBKA+u?±>d~f?£ÞBKA+u?ïõ˜ÝÔSv?FgÂö]œ$?TÎD¿Í2í?FgÂö]œ$AGN4FGL J0539.7-0521c¿á÷œ¶w¤À2_5ŸôýmÀ9ə~Á¦ÿÀ;T²ò03¤@¶FÉ)@0Þ@'—?ÑáõRýÔ?äŽàØóL@-d"¿G©?û½DC¦É¿â†¤^ïy ¿ÑYƒÿÔa¿çãW=SŒ¿îýÄupÅ¿ïþï~þbÇ?ïýß(ïãRAGNbcu3FGL J0539.2-0536TXS 0537-052?æe¿8©X˜?̄"Ÿƒá?Ó4Ž­NÐ?̄"Ÿƒá?ÚøÁ33V?ÌYÝKË¡?⃟@ffU?ÌYÝKË¡?ç>ӈ[aX?°'8:óµ´?тXïI=P?°'8:óµ´?ÝΏ¡{Ä?¸©‡U!Ú?áó¸/B?¸©‡U!Ú?ÓÀP;<þ?͈V¡ÞrÎ?æøWâa?͈V¡ÞrÎ?¶'&Å·?»89±–TZ?í=¿ªi?»89±–TZ?ӌq¥+?–?¶´²#/?æ9Ç-j`5?¶´²#/?ˆçzéyW?€c˜ÝÝBr?ïœbƒUò?€c˜ÝÝBr4MIXED4FGL J0539.9-2839?쫦ÕÑÀ;FE^®âÀ8ÜhìR¤À<:kHM@æo¨"µ@jnü7£?¤àš_]u?¼£çü(/@IŽ|/%‡@³puÞÔa¿ÒԽ렿æV¡ÍD¿é®/RÓâk¿êýDcÝ*¿éÒ%Âu:¿ïÿùëñAGNfsrq3FGL J0540.0-2837PKS 0537-286?ïýf;âóï?+í™-ˆƒX?4Î tí¥N?+í™-ˆƒX?ïöŸÞF
À?R¹ŠËñ?RÀCýZß?R¹ŠËñ?﹋K6?€U2óÛw?-HrÀ~?€U2óÛw?ïöÕîÎC3??ý¹ú|U?RT"`¹éo??ý¹ú|U?ïþ].Ì¿?&E72Ù?*._æ® É?&E72Ù?ïÔMŒÐ³a?ÿ"Ú˜±?uÙ9–Fwa?ÿ"Ú˜±?ï Æ¤ó ?Šµ%¶ÿÎ/?‡ÎVµzgÿ?Šµ%¶ÿÎ/?ïÆíï/Î?p.ĖÏ?|‰t†XTñ?p.ĖÏAGN4FGL J0540.0+1209?àã']ëÀ#©QçS`ÐÀ:MY0ó½ÒÀ<ږ¹ëI@1tÅyÇA@b‹°¢Ê›?ÁÅ«âqz?¦í´£á8?ç*êßÝJÉ?ÿêEko׿ß;ž¼™#¿àÇ÷°¦%™¿è""j«o…¿åÂù¿ŸԿՏF¹!õ¿ì©«àn[AGNbcu3FGL J0540.0+1208NVSS J054005+120955?ïùÖv*˜?8·ø5U\?H§å(Ì),?8·ø5U\?ïïBœÌmÆ?`­î½óÎ?`½c("yô?`­î½óÎ?ïâ-±×?d¬Ùşx?mÒO0Õ`ö?d¬Ùşx?ïï´q¿¾?F`'ìWÆf?`ôK°œYV?F`'ìWÆf?ïîŸÂ7?UQ ÇæR?a`=¦(q,?UQ ÇæR?ïÁVÊ^?'Ù1]eÎË?9qs‡L•?'Ù1]eÎË?ï¦ÞV•–ˆ?"œjø¶$?†Hjay•ä?"œjø¶$?ïl2'=H¥?',S!e'r?'y­º¹i?',S!e'rAGN4FGL J0540.5+5823¿ïÿ䞝@,‡îõìÀ9·É°¸šÀ<1µ°P•D@ {Md·»?ÿ4ùÜÐP?° ÄÍ¿ƒäª
I…?×^ëîù@ê6êø²?ïªÏL¿µTÂ$'Q©¿æyWÊÆb¿Öt{/PP¿â*@Õ³P¿Á6"f\UkAGNbll3FGL J0540.4+5823GB6 J0540+5823?ïýÖÿo{'?!»Ø'…ÀH?1H²T¼>?!»Ø'…ÀH?ïð¶Âìœ?`ôË@(C?_ԒåZ˜>?`ôË@(C?ïõÛÿšªf?Z 6®.'?THQ[ã¼?Z 6®.'?ï髙#=?QÈÄ
£ m?fTf"øŠÂ?QÈÄ
£ m?ïúv¢.ú¦??—XçùW?F%x	þèÈ??—XçùW?ïÁèfAŽ§?…´1ƒ,[-?Ìõær?…´1ƒ,[-?ïïhï
lô?rŠîHÀÇ?`—+ì?rŠîHÀÇ?ïÌ"	Œ"?g"SñTþ?yîûQ÷½?g"SñTþAGN4FGL J0540.8-5415¿ÕZA"öÀ?ڄœ²RÎÀ9Ö­'¿À<0'5G	ª@P®äY†Y@×¢~D©}?·…ß'˜J?¶vÙ{0øÆ?ù¸ÞÙ>Ë@üwÒÊgÃ?éÕá[Ð
¿àÚçœr<¿éW°´hR¿é
Öøj
¿é–š«èP·¿Ó3«¾Š>ÞAGNfsrq3FGL J0540.5-5416PKS 0539-543?ïþ©An?鉻í?%o»Ó7?鉻í?ï÷:¡¼}Ê?R/°c^ðã?QŠ¼4Ì?R/°c^ðã?ïÞ²¿?o!ãÙôr—?p¦··ÙJ?o!ãÙôr—?ïÿ1ÅÛþ?	])N†?™Ìg"R­?	])N†?ïý~Žƒïl?.I¤w©(J?4‰ËAC¯?.I¤w©(J?ïÛ±P¼ÓR?A,å£Ï?r'W‡yO-?A,å£Ï?ï³"'K?ƒt+ã>?ƒ7~®žó?ƒt+ã>?ïüüٖ?*ý`4.&?84…?&?*ý`4.&AGN4FGL J0541.1-4854¿Ó1Ō‰HÀ?[ÂôÀ;Jh˜À<»ú`ƒÎV@ I'ˆ°é?þláłU°?ʧ6eAÎ?±ç0Ñ.0j?æ£ø'Ä@Áp¾0a?ïà¿ÞQÚh¿ã8 7­ì7¿×@-…öú¿æûm"X9? ýÜåÑw¿éÝ}‰˜š–AGNbcu1RXS J054106.1-485408?ïþʶG$W?.˜óz=?#T™0ÿV?.˜óz=?ï÷ûWàÍÇ?P=Óºá?P	P£EƏ?P=Óºá?ïóòÅÒ)%?`plÂ%Ÿç?Xt=q'?`plÂ%Ÿç?ïþ™Fž±?:ñ¨¾ñ?&k•Î-[?:ñ¨¾ñ?ïÿ7jûK?T©ò©j? ¢mä|?T©ò©j?ïٓ†Hó©?~С¿/?s6<çäà?~С¿/?ïécÖ`–»?r½½Ësx?fœ)rm0?r½½Ësx?ïûD˜Ð	Ý?7rïNŠ?Bí4dåZ?7rïNŠAGN4FGL J0541.4-7334¿Ó‡±w†ÊÀ>Þy!°À:Îނö À<qÏI~Ï@D>·Ë³È@o?¾[ðÂ?ÇÍ|µˆ7œ?´e8>ŠÕ?ìÌxžÍ5'@¹\Øs?îñÓ'é|¿æPµà!=g¿åt!N¿ã%€Uпæ¢'Õ¿ï÷z?·%AGNbcuPKS 0542-735?ïý&O†6L?*xáNš¬?6ͅ2‹‡:?*xáNš¬?ïô˜C`Ûk?S¿àã'ª°?VÏyÄùÙõ?S¿àã'ª°?ïîK䞿b?`Oã'>
?a´‹ÛÅ«?`Oã'>
?ïïÃÑóʊ?@àY3Օ ?`<.4íÕ?@àY3Օ ?ïû_‹&Õ?8¡DÒ<À?BÔ*þaƒ?8¡DÒ<À?ïØX£§†å?tæ"à‡ñ"?sÓ®G¹m™?tæ"à‡ñ"?ïçÉÙ0?qã8®y"÷?h6'‰Ì?qã8®y"÷?ï©i؃0Ä?p IFP‰?…¥‰æý?p IFP‰AGN4FGL J0541.6-0541¿íÍò¨mÀ2üÞãOÆÀ9®Äjþ{œÀ;]±÷^pÏ@,¤ÅFƎ@ÙEnŸ?ȪÚ3½œ®?Æ6·L2º@	zÓõ@S¬–¡l¢?ïþVèD!˜¿à.ñàW™¿è:#aÔÜ¿êsp-…¿ïçæcvÇÝ¿íyº×AGNfsrq1FGL J0540.9-0547PKS 0539-057?ïïþ((ï?^®Ýãrn?`سÈÃ?^®Ýãrn?ïß±€ëù?˜TxçÃ)R?	ÉHó?˜TxçÃ)R?ï>_ÇÄWç?Œº'DÏ2?˜4g+?Œº'DÏ2?îxO‹È:?‹ ¨Cºò?¯{Óàm?‹ ¨Cºò?ïsØX,x?"'5X7µµ?'"õk?"'5X7µµ?ì¿]8¦v?ƾ÷×½k±?ºí:ÌQ?ƾ÷×½k±?éíY©{?´MÔÉ@\Y?ËÄKš™Z?´MÔÉ@\Y?àNŸÜes?µ™ rÎ??ßbÀG5ý?µ™ rÎ?AGN4FGL J0542.4+3547c¿àµx{æ"@ÔÏr™À9{ÿL{ٕÀ;/(«ôž@ý~®Ü¡×@cwá¸í?É©½(?^?lj£Aãû@gÀôQv?ø?	ˆ??ïÿÝ/ñ_S¿½èplN²Á¿é}ž¼C¿çQ˜Wz:¿èªŒ€¬bÊ¿ïý¸È3
AGNbcuNVSS J054218+354149?îÎ7}g+U?»}
x?£ˆ&®¹?»}
x?ê_þ^·"?ÁÕYáü<…?ƃð…!µ?ÁÕYáü<…?îÃèçNr?‹¯_Væ?¯ÃÁu֛Ù?‹¯_Væ?êÛcâ!ž?Ÿ:;rïL.?Ēsàwy‰?Ÿ:;rïL.?æÍΐ­s?Ì3†À#8?ÓúdbÞ¥?Ì3†À#8?Çæ6¨ô?Ë8ÇÒgŽ?ê`2UùÃ?Ë8ÇÒgŽ?ãwд8w?»š9Û «?Ù^—ÿ?»š9Û «?Ðtr½%©¢?¬&ÖÀêð?çÅÆ¡m+/?¬&ÖÀêð0MIXED4FGL J0542.8-3458?ÔâäசÌÀ<u?|ÌÀ;§W>«6zÀ<åÄ÷u³@ Ó,nÈà"?ý<ÙTšŒ?Ѷb'œOV?¶wÁ­‰æs?ènò&"©x?÷p'¢Ü8{?àÈ'Kžd¿ãÏi_?*¸¿·ýÌ^'Ýh¿àG>îRX'¿ÔÎÄɞ¿Ü œ'­ýAGNbcuPMN J0542-3500?ïþÐU‰Š?½ð wÿ¼?"ú±Ÿ
c£?½ð wÿ¼?ïñF=É[¡?a
϶¶?]s"†îÏ?a
϶¶?ïï	Zœ®¢?_~&'°8?`ö¥}neò?_~&'°8?ïïVYÓÛà?F¡¶`èíƒ?`©¦nŸê?F¡¶`èíƒ?ïÿ}•pÚ?BUkNˆ?ðJµcý^?BUkNˆ?ïÉcÆÃb?ƒu/"Þ˜?{N>Jzº?ƒu/"Þ˜?ïížæ¬ê&?n(¶IÖøE?ba`ÔJ'?n(¶IÖøE?ïªÕ»«4?v!;šýö$?…yJ¥—?v!;šýö$AGN4FGL J0542.9-0913?ïäèuÛàwÀ3^rÚ/­À8Óp]`-gÀ;*[rÏ*@¸	FOÆ@×üMÃØ?´ìÈÀ£ž«?ÄyÔttF@¥!Whœ¢@ãðŠD?îÛD)$¼¿Üø,AQ"¿é¡Þ¹q¦¿æ# ÄS¿êÚ÷½'E¿ï´~!nÑAGNbcu3FGL J0542.5-0907cPMN J0542-0913?ïáöGÍý'?l Ü­Á?n	¸F %ä?l Ü­Á?ïå}Z?kèù;ˆF×?jà'°ú¬U?kèù;ˆF×?ï	<7?"ÄäøS?ŸžÞ~°G!?"ÄäøS?ïŽôwyÖ?m¡×ˆîø°?ŒBý"!Ša?m¡×ˆîø°?ï&\;ê$?œkÔ¢Iº‹?›4xœb»{?œkÔ¢Iº‹?ï~Ç#s*M?›XME™l?'ŒsLp?›XME™l?èÁQ¼`C?·Èh'Gç?Ìú¹~óÑ?·Èh'Gç?ëø•ÊO´?¤5↏ª?À«ÖÁ1?¤5↏ªAGN4FGL J0543.9-5531?í°ø;C*«À?z]9–úƒÀ8´ŸVqüÀ; L?b@êˆü¾W?ú'åÂg=?¦ –R?±Íߢú@ìÿdύq@)øH¦Œò?ïÍϖ«¨¿¿Í­$Ù¿ÙW97Y2¡¿Ôh>Ã4G°¿Ûï?='—t¿Ùâöúó¦«AGNbll3FGL J0543.9-55311RXS J054357.3-553206?ïýó	ïºZ?&N‹'³Ê?0g®î§ß&?&N‹'³Ê?ïõçsþ:¿?Vl<€B<\?T1ÈQ'?Vl<€B<\?ïáéão6Ö?r\ˆo7_?noÌês?r\ˆo7_?ï÷þ™ùf?:æõ33ÿ'?QÔ1Á£¹?:æõ33ÿ'?ïýUÍß?*¯†,<™J?3¨=à–?*¯†,<™J?ïÙFÔ¶â?x˜Ë̆??st\štÜ?x˜Ë̆??ïîaòA?qÍ`c̑ì?aúêÿ?qÍ`c̑ì?ïìOSÐ6º?RHI°Ñ+E?c°¬3èÎU?RHI°Ñ+EAGN4FGL J0545.0+0613c?¸âîë¦CÛÀ'qýiôÀ9ì0Ûj'À;¡[wN@ź+µe@ñèæ?ÎUlƒ‹æ(?âÕýÞâ@†I%ÿÃ@³ƒJLÕF?çÕ7Ÿ©~¿Êø›‡°c¿ê¤0ÌP¦¿ð?ð¿æbb™RLAGNbcuNVSS J054529+061955?ïµ1²w?®ðe"qõ?'³"sr—?®ðe"qõ?ï Wqè
ý?—K"4![?‡ê#L¶?—K"4![?ëv"šó¥˜?¬ÂÅR~(Ú?Â%í"1iž?¬ÂÅR~(Ú?ïï-=r?[$gÂÌÀ?`ÒÃ'ýµü?[$gÂÌÀ?î'ÉЫ:?²œ¦'ª:'?§ÓoÁ=~d?²œ¦'ª:'?èRF…£?Ò4‡˜Ý~m?η²çÑéu?Ò4‡˜Ý~m?æ¿ói)öZ?¶—ȦOõ?Ҁ-¬L?¶—ȦOõ?ìåª4?¹X¸]<Ã?¸Ñê¯;
{?¹X¸]<à AGN4FGL J0546.9-2206?ìg"þÀ7 E®_úÀ;~?SÒåìÀ<̍‰Àß@!
¯Û¥W¾?ý¥È–Ý&·?˸é?©"ô›ó»ú?⥡õ¿?ÿëWã俗…"úÙ®?ïùõß덂¿ç¿Àéz-¿Ö—
]¦ú*¿ã/5b7'£¿½ÿ¹3<îHAGNbll1RXS J054656.9-220500?ïþ˽á«	?á-n'O=?#D ¤@À…?á-n'O=?ïóÃVVxÞ?ZÊÙ9J?XyS¨D"q?ZÊÙ9J?ïòä=o?`!Ê,n?[Ê6¡Pþ?`!Ê,n?ïñ¼÷dR?CtËm?\†@Ú?CtËm?ïÿ&óx¡ì?syZCQ?!"ˆCFã?syZCQ?ïËÌ&‰¬'?€´óè{?zìºyË4?€´óè{?ïó
²Ve#?h÷WãfN?Y䛻©Ú?h÷WãfN?ï»SÔ¤˜·?q'ã]©œ¦?+
Ïúš4?q'ã]©œ¦AGN4FGL J0548.5-5218¿ãZèåÝÀ>‹¨çv°À;dÿÑÜ×À<àNú9¢@63Ÿi½3?þ^Õ®Þ]?ÓDE>Îqè?Ý\Šû>Ë@ØÌ<"Í@à\Õîßq¿ïÿ¾…{ª?ïâFj^?Çi^GG¿á'V½•!¿ë•ö¬š'^¿ïíFõ‡ÖùAGNbcuPMN J0548-5218?ïøsé‰?PÆGØrѐ?N3´Ê(ƒ?PÆGØrѐ?ïí(¯Ì‹ß?brpyQˆ?b×PY˜ü?brpyQˆ?îá=k+®@?'p'¬?¡ì)Li5?'p'¬?ï©ÊV¸?j»Ôïëf¿?…~íÁ›?j»Ôïëf¿?ïߘ4oÖ?oyìK‰i?p3åØZù7?oyìK‰i?ïÁd"—‡y?"U™-›Á(?M½˜¿cŠ?"U™-›Á(?íÅÆøfGv?¢¦°ÓMî–?±ÑÈ<_ÐÍ?¢¦°ÓMî–?îÐðbJšO?'æ?(x³à?¢ðùß¡Þ?'æ?(x³àAGN4FGL J0549.0+3258c?á7Ý.V@Ä{'W]µÀ:e²ÑyøÀ<Ô€ö@ ύ3YÉ ?ÿ­*:f-\?ĚS¾C4?²þ½à ¿(?ïïãB/$†@‹99\˜?ìÏt…
?í÷y´!]?¨]‰a×Ð%¿ãµÁM<ɵ¿ßЍ]b²¿Þ•Á}ŽK2AGNbcuGB6 J0549+3258?ïúši3†{?=}­©¯t?E–Zá¢e÷?=}­©¯t?ï×
À)r·?†¬€ç?tyç'I?†¬€ç?ïìfÂE¤?eÓ9nÁ?c™=´Ü*?eÓ9nÁ?ﱤÏq†š?kpwÕq?ƒ–Ì2¼¡w?kpwÕq?ï÷ädå?Fòï'ÛZ-?P7ø'Õ"?Fòï'ÛZ-?îÑ(ÇmŒ?¯sW¨—ë?¢ísÊøÃ=?¯sW¨—ë?ïÚç}äB›?}MV]üRÖ?rŒ@ûPÎd?}MV]üRÖ?ïyÁž+¶?ã­i#<î?œPÇÇN?ã­i#<î AGN4FGL J0550.3-5733¿ÜV y®ºÀ>´üvÄÀ;‡‹z&À<§—…Ã#@@§c±«3@¸¤ÁëÈ;?Â{A–£E?}s±¸ç?»i"d O@3Yàqs?ï½|˜%¿Ý¤q"&À´¿ç>A¹Þ³¿äz/ ~û‰¿êBª¿±±=?ÛÒHÂf—dAGNfsrqPKS 0549-575?ïýG^Êw?HOÇm±A?7ýÆàC'Õ?HOÇm±A?ï÷ªÕðÑ©?RÒð÷eÞ?PªSú ¿?RÒð÷eÞ?ïØÇã"5?|ÿÑþǒ?sœu¡¬µn?|ÿÑþǒ?ïýõ9J?!¼÷O?7¾ š¦?!¼÷O?ïúLˆú?F$›ž']õ?GžÏ9þSì?F$›ž']õ?ïÛU¥	J"?6Ê9Ct?rU-€**¡?6Ê9Ct?ïÒfûÈÉï?|º,fí?v̂0èœ^?|º,fí?ïô'äý"ß?Fd×DÈÐu?VÚ6Oñҏ?Fd×DÈÐuAGN4FGL J0550.5-3216?ל´è:ÎÀ:.—á2µ_À:EÂHåL À<eg?ª9û@ 2x'$"?þÔóý">6?¶™÷']ῚÎL‡JÀ ?äØ<l—ØÏ@–ß~*R¿ÁaL ?¿â™baÉô€¿ãžë}'ü¿ÃøÄwhÂ6¿åø£_–¦¿È¢›[e¬AGNbll3FGL J0550.6-3217PKS 0548-322?ïý€ïSµ_?"µ`	Dƒ ?3øƒüý«¸?"µ`	Dƒ ?ïö£M!›Ü?QóM›èt
?R¹eNÔÈp?QóM›èt
?ïõhJÓI$?L
zÜi…a?U/jvxˆ?L
zÜi…a?ïôf}H¼C??—Ìç,%?W3kÇÊÀ??—Ìç,%?ïûx±9ì?6''|ʾ?B:T©WÈ?6''|ʾ?ïÛ¨Ô†;?téç~D?rs«›<B?téç~D?ïö{¶'?brˆtž–?S"†1îG?brˆtž–?ïÔí{ª+ž?bÖT)\Θ?u‰BGÆè°?bÖT)\ΘAGN4FGL J0550.9+2552c?àZ&|ä¿â"Ùîô?À9æã3@Ÿ-À;\€¸!D@q`-…Ÿ?þ£Ah€?ÔVK¼J?ä±il«$@'Á¯bY?÷îÿ&¼,¿ítD
õ?í®¡žJÙB¿ÞГ@d8¿äì;\Í`q¿ïüá1ޟ]?ïzô}jäÐAGNbcuNVSS J055119+254909?ï`'‡ëX?£tEG=?œóï¨#]?£tEG=?éE0άù?Ç9gEŘ6?Êë<ñÅL?Ç9gEŘ6?éK[¬×õ?«¶ëüX—?ÊґOü -?«¶ëüX—?éH;Ù)/?¬–Çq?Êß´›[C?¬–Çq?éw *Wlx?Âê¡Ô¦Šï?Ê!V¢N?Âê¡Ô¦Šï?ÆœkARÂ?Ê?·»m©Ò?ê{Xå/«P?Ê?·»m©Ò?á
ãúç	?·¯¯ª* ?Ýä9â
1î?·¯¯ª* ?Ðw^'Êìš?·wÐV
5š?çÄP쉳?·wÐV
5š(MIXED4FGL J0551.0-1622?Á½ÊG<«À4ŽùÛ"ÐåÀ;jNÕP)
À=<±¥)@z8MNgl@‰üpy?Ôa):¶à&?ïü辚Úâ@n'"šV@Ÿêw­‹"¿ïè—8å?ïý2%9þ¿«s€]æï¿æIàô¡þ¿ì³·RDÌ¿ïÿæÀ
AGNbcuPMN J0550-1621?è²Hù)]X?̀JWÎ?Í6ÜZŠ¡?̀JWÎ?ï´²ˆ—¥?‹÷DÃÊÙ?'Óx(ØÖ¹?‹÷DÃÊÙ?è8' B?°ÍËKY?Ïß·~÷?°ÍËKY?î9Ô=b?"z,Yá¤?¬o'»M÷Ä?"z,Yá¤?èªEAa?ʨ½·Ð^?ÎVêûêz?ʨ½·Ð^?îûß·«É?² õÌŒ? B	\p?² õÌŒ?àåï÷°am?¹DP£×?Þ4 Ÿ=%?¹DP£×?è_nö‹jµ?¸9}ôÿD9?΂D%ÒU+?¸9}ôÿD9AGN4FGL J0551.8-3517¿à~kÊö«:À:¿ÿ›V2<À;_ø[ÆÐÀ<®}1"Š@7ÐVD/Z@80êÄ?Éãã¿­€¿ªÕ!ș?àèøFΫ@û‰"Óê¿ÐÊaÛ<Q¿èsáÿcøο蘰C)J¿Ò·ÇíiûF¿áß& {±¿ïÿž´JAGNbcuPMN J0551-3515?ïýyqSæ?%WÝp,Ý?44u*ëÃ?%WÝp,Ý?ïöM'Ðæs?T§´ŠñÁ?Sdú¾h)6?T§´ŠñÁ?ïïŠþåèk?ZÔ-Û¯º€?`u9œ›?ZÔ-Û¯º€?ïýºcú·}?à	`®©Æ?2,áÏa/?à	`®©Æ?ïþ|4%n?(9¿UŸ®?.(<	W;"?(9¿UŸ®?ïÙÆAº¬Ü?~EÀ˜ÿÈO?sßA–
Î?~EÀ˜ÿÈO?ïç{Òh?rufL4V?h"úÅÐr?rufL4V?ïîºjÊy5?W(;	¢µ\?aE•5†ÊŠ?W(;	¢µ\AGN4FGL J0552.4+3755¿ïHsò@#Ü@G¹EÅÀ9£4EHßÀ;º]éÀ"š@n¬`@¡59°€?Á—O Ò?Á2ZR½?üzžF§">?ÿÿa¨â¿Ðqm*¥Æ¿à)û|ÀÙ¿è¤@¼ˆ±ë¿åPŸ?J螱Áƒ˜{¿çWÿñ<nAGNbcuB3 0548+378B?ïÕñѾùû?ƒCB¤Z1ä?u(&I?ƒCB¤Z1ä?ïŠîþÐÕñ?'?í¦˜!ù?D@R©»¾?'?í¦˜!ù?ïT´:æ†?ŒPë7Ã|?•inVëaG?ŒPë7Ã|?ï#>Q°ˆ?{´}?›˜5˦̓?{´}?ꯩ·…?ÀuVùáØÎ?Æ…AY!ë?ÀuVùáØÎ?ë´)5at?ÀÐ!|7Å?Á/[*{²1?ÀÐ!|7Å?ç‡nq«Fž?¹Æ g,ù¢?Ðñ#©rÄ?¹Æ g,ù¢?èY,A&'?­ª;Ü['?ÍʛNûe¼?­ª;Ü['AGN4FGL J0552.8+0313¿áÖÈõ¸åuÀ&ñÖ1riÀ9Øe8hýÀ;eQ‡²‰@q¡L–[¢@Fü"û­‹?Ç´°¶Áš?ÑàZ]āO@
ûÅ<@ÿ7VÙUœ¿×í\¤Æž_¿ß&H>2?ÿäÛâ…ï¿èòÁˆËëü¿å«hÎör¹¿ïþ3AGNbcuPKS 0550+032?ïÓ·ÉÊ'Æ?­†ó<Ä?v$
ݙ:?­†ó<Ä?ïìa¼wXì?d	Qþqà?cžCc‹Lp?d	Qþqà?ï•v5´?'ØUþ'Q?ŸM]?'ØUþ'Q?ïáÓMU¯p?W§(¶ ?n,²‡ôx?W§(¶ ?ï×B®?1Þ?vƼâz?t^¨Úç±?vƼâz?ï ã2rvž?'?ñë;ä?‡Ç3R4L°?'?ñë;ä?ìÕ«=äo´?§<J•Öp?¹R¦$´`?§<J•Öp?îy
ÂÉ
B?›1M䬖?¨oSÕ')ß?›1M䬖AGN4FGL J0553.5-2034?ìÍ¿ª5¯KÀ5ž YžØÀ9Ýu&Ê;À<­ê‰v6@~¸w«?ü9 4¾M®?·
´ÉuÕ?Ã׎\Nµp@ÿW}•@¼E˜•?ïüÀO(\¿Úx6<Òï&¿Ñ°'#Ùy¿ÝóÎCoks¿áè–!?é¿å[Û]‰HAGNbll3FGL J0553.5-2036NVSS J055333-203417?ï÷̶¬b?R ãt¸?Pf'Ÿï
?R ãt¸?ïìzD%?`iF‡z;?cü…ð‹?`iF‡z;?ïÎãÂ^V?sÊcbé?Ý?xŽ|—A°é?sÊcbé?Ý?ïÁÎ4"i?ZÑÜõ"Í?rÖЃ©?ZÑÜõ"Í?ï¾óßË?€GU÷š_?€C:rËD?€GU÷š_?ï¯ã…K	?ˆî<R#Šà?"¬QÙ?ˆî<R#Šà?îá\ù"?¡þÀ7Xªé?¯ïÊ0må?¡þÀ7Xªé?îîv¡ƒ..?"†¬…F¶?¡•è©?"†¬…F¶AGN4FGL J0554.3-1009c¿ß!q¦3[À1<yÄ<hÀ9ÖÁ['—À;¢˜¢ô@>ñŒõœ@W'"¬Ó2?Ì°rùòŸÅ?Òc¿m@ë_ïIÏ@☡!"e?ïû%|'¿ÞôÔRÓ«¿ç¸}õÏ$–¿í—'"Yœ)¿âùƒ¿g´o¿ïü`8NûçAGNbcuPMN J0555-1002?ïêÝ
 "?b°ÝE§ä?e"õ²!
t?b°ÝE§ä?ﯽX¡½ç?ˆ\°½Êà?"©Ì'Æk?ˆ\°½Êà?îæÞûðÉ#?'Þ_Ê|?¡'@ómÔ?'Þ_Ê|?ïw¥?·rj?r}¸èÁVk?'X2zË?r}¸èÁVk?ï©j'΁á?†:¬Ís¨Ô?…¥[>¡Á?†:¬Ís¨Ô?íÇ>ŒœtÚ?³/­`@Ÿ'?±Æœf3®?³/­`@Ÿ'?éb"ÃéB?²jlAN?Êwtð[¶ú?²jlAN?ë,Wïn?«:éòÕó?ÃOê£øBF?«:éòÕó!AGN4FGL J0555.1+0304¿ë
ÇÇæoFÀ&¬ÿ§ëlÀ9•'ußÀ;;\ºëù¹@"©	#?J@X$¹ó¬5?ÒXDЩ*?݀£(Ž"ƒ@kE®_ú<@Üƒ#5?ï½<Á§TÿÆ?¹éÆ,Ë¿êz73rô¿êm3t¡'Œ¿êõÀv}4ß¿Ò¶žb+CPAGNbcuGB6 J0555+0304?ï×ò'?d­<-Á¥ð?acwõ36!?d­<-Á¥ð?˜½?•^†zlÏ?¹8dX@Ê?•^†zlÏ?íÞ«Ý?£OÝP8Ç?·é
©:ò%?£OÝP8Ç?îY¨ô'ž	?ŠÃÄÊў8?ªepµ.Qu?ŠÃÄÊў8?ï¡e¶K1?–Ü	3c?‡¦''Lk¬?–Ü	3c?ë"ù@ëz?Ê·>cE¨3?ÃtüRò?Ê·>cE¨3?é8q°"Ó~?°À4w¦·?Ë9=°²?°À4w¦·?ޟ­ÌÎǛ?¹¸£R³‰¸?à°)˜œ2?¹¸£R³‰¸MIXED4FGL J0555.6+3947¿Ü†_£@&7yéÐêÀ8ÃÑv¹À;™Ø)!az@—v³·X@-µ@å£?¯ó–Kwx?Êe*&D7g@Á+àŠð@$5f¿&Ç¿ÛMÓÈi½¿ã½R ^DY¿ê¨ðN²¿ë-€@Ø¿î9Ìzd¿ïÿþó…õAGNfsrqB2 0552+39A?ï¤Ù)ì&s?ƒUÝ0¸?†Éµ"öc8?ƒUÝ0¸?ïÌëÍ|?Ôí?¤~Ò?yŠ~0K)?Ôí?¤~Ò?ï
¦ŽÊˆ¥?'õ*÷Àåe?žK.!‡m?'õ*÷Àåe?ïã×;¡Òß?T×ᚻŠâ?l(Ä+Ré?T×ᚻŠâ?ïgþ4´ù®?ù2éZ?"9g¨üP?ù2éZ?îµ)þ‰»ß?±´a1æZ|?¤­`@)?±´a1æZ|?îe'•?¢á¹¼ mŽ?¯Ù­šÇg?¢á¹¼ mŽ?ïòÖC?ŠýuÌé?ü¿íi›?ŠýuÌéAGN4FGL J0556.2-4352?åƒPàuÔ¡À;ö:\`‰À:&þìɹÀ<G|¾—ä@Á8jª™?ýª½þÓ°?¹œµØ¿tJ?ÄZã»Ñ§Ó@	®¢?Zˆã@	茿ð?ð¿ÑÄLá<P¿áânÁŒ¿ã©LŒ ¿è"¤o¶AGNbll3FGL J0556.0-4353SUMSS J055618-435146?ïüsJlú?<õNÄ˂?<c5©4ÿ?<õNÄ˂?ïõl4 _u?Tüï(f+{?U'–j
Åâ?Tüï(f+{?ï­\i¸Uq?†Nô2Va?"¨å‡›Ï±?†Nô2Va?ïõˆ¼7å[?<T2+~7ƒ?T?<T2+~7ƒ?ïú×)Б†?B;!ĺ©?D£Y@°Û?B;!ĺ©?ïË·ÂJ`?…w=ö"?z$Üþ·ð?…w=ö"?ïƒþ¼U~?‹Wùç>?:€TZ<?‹Wùç>?ïÚ<¤¡	¥?c®Dk…?r᭒žup?c®Dk…AGN4FGL J0557.3-0615?Öтéÿ¹À-ºIÂÁ±À:''¡WÓüÀ<*ý"û|ä@!7œÏY?ÿ—{ž?ÂàU*S懿t¼™4*:L?©¦^ÄԎ?ÿPûB÷?Þ­¥,tÓ¿«ƒÕü»Ú¿èí±´B'L¿Öð½!´Õ¿á,ï¢9Ñ2?²¼ŽŽ#AGNbcu1RXS J055717.0-061705?ïüJÐw•ý?03¹ÊYØ?=©~gøà?03¹ÊYØ?ïôgÊ$âõ?Tᙢ½ß?W0kcÃwM?Tᙢ½ß?ïñгñ­?MǼuUïì?\^šWõ´?MǼuUïì?ïïéz£Ä?C|âïD.?`…øÜÛó?C|âïD.?ïûô†éØe?5pniªDh?@-ã€Ùy?5pniªDh?ïГlj»?'*œû¿¤©?w¶IԐŠ¯?'*œû¿¤©?ïï7¶?gۑ²ÙªU?`æé·ËÕ?gۑ²ÙªU?ï°GCò"S?pÓ£ƒ
â‹?ƒî.òˆÕp?pÓ£ƒ
â‹AGN4FGL J0557.6-0721?ï¦KXÃæÀ. ù	kºÀ:ÔdÓ¿/UÀ<@Ñ0ߛÜ@!GÝcp?ÿ¢ºtÛt/?Èêo_‰Rz?Ê¥Þ©÷"?ÉU·­¢@ÂÌå¤?î¥ÉB©É¿Æ3IÃîVà¿ì"֎ín-?¦ùQÁ¿ßË¿ñò÷¿Í9б3AGNbcu3FGL J0557.7-0720PMN J0557-0719?ïÿru­?½/º+öO?1´6¸Ù?½/º+öO?ïõ®ØÅÿS?X–̨»©?T¢NË
?X–̨»©?ïá·0"ƒ–?y]ôÌ¡ø?nHÏn<ž?y]ôÌ¡ø?ïýÐÊL-Å?(õÛ-¡?1y­S͍*?(õÛ-¡?ïþ‡6ŒüJ?.EO$Çñ?'Œ"\ÀÛØ?.EO$Çñ?ïÝ­ÌÍ?€7šnÖJn?q)ü˜Óß?€7šnÖJn?ïØQ«r?"¾Ë¾,?s×*d¨¯5?"¾Ë¾,?ï÷،§ s?Céò
C»×?PNæ…7\?Céò
C»×AGN4FGL J0558.0-3837?ïf™UbCRÀ:mYėtÀ9¢&¶ÁÉÀ<.‡'§
ö@ʹø´²$?ýnz[æ±?³Ò<^'A?¬Ü	֘}?ù&رÝ]@4hwä?íCy1DEª¿â$;H«j|¿Ü»µƒ+ß¿ÛÕгÚ
¿Ú/¡ãêöƒ¿â¤®ÀÈ1²AGNbll3FGL J0558.1-3838EXO 0556.4-3838?ïý³bԜ¶?!ý>67^$?2déå¤(2?!ý>67^$?ïöÅWC<?T·¡É#*?RuQƒèã?T·¡É#*?ï÷˜¬´©?C.èbX¹?PÄÎÏÑüò?C.èbX¹?ïì[¶Sº?JÚým_Â?c¤àWj¶\?JÚým_Â?ïú9ÝÏÝ?<"ÂðɌí?G‰W.½?<"ÂðɌí?ïÕÿo?€?Hó÷?urtp¦?€?Hó÷?ïîE‰æ·ô?pfÚæ§%?aºvYà³j?pfÚæ§%?ïÉæeÐ~?e؆!î@~?{Í8ò€·?e؆!î@~AGN4FGL J0558.1-2859¿âŒ}|W"À7™0ߛÜjÀ:Ñ]ÓÀ<šz¦]Í@Œ›Ág
@æÜB‹–?˒ºNðÔ?Æp˄£=\?ø™åi{Ĝ@Ç9©Ml?ïü›ÇqC9¿ã¥ÞPݾ¿æ4Š¡.8x¿åÖÇAÈwS¿ïüõ$®5¿ïف±E‡ÊAGNbcuTXS 0556-289?ï÷•]tÐ7?HÈ~æ°×?PÕD°«#p?HÈ~æ°×?ïñt¸þR›?[Ödâ>	a?] fS?[Ödâ>	a?į̈LÐ˜?p‡Ov'' ?y«Ù›êè#?p‡Ov'' ?ïÓ$a«Ž?Xâç ø…{?vmÏëi"?Xâç ø…{?ïô~ªTý³?SêV÷Ó?W«$Š9±?SêV÷Ó?ïɌÌÉÿ?|
ÅÛ¬è?{9šz8B?|
ÅÛ¬è?ïGÆ´{G?]¾ƒ%<d?—<I-?]¾ƒ%<d?ï;™Ê?ƒR؋cK?œØ$"¿?ƒR؋cKAGN4FGL J0558.8-7459¿ï\nW˜åŒÀ=†r!…‹ÆÀ9҈u"ç[À<U¼ö•óó@ÚJŒÁo?ÿ¦>{f?µì>A¯!ì?±›!ô›?ûHÆÆ#@ê¬0Êù?‡'ÑTW+¿ãf$!Gx¿áÓ/M= ¿Ü+%Â1h¿âG¦Ý¤áK¿åW¥£"ŸAGNbll3FGL J0558.6-7459PKS 0600-749?ïþ¤¼"/?€Og%GÑ?%´>ˆ¯[?€Og%GÑ?ïõ?•R'?W°$ØÌê:?U€Õs&¢³?W°$ØÌê:?ïøд

Z?[m 
Š~?L½0¦˜x?[m 
Š~?ïöÍogŸ?8ÎÑÎR¾?Re!}¸Al?8ÎÑÎR¾?ïþšF4?#ÞÆn--o?/a	z¶K?#ÞÆn--o?ïÚô9<%?}»ÌáMïî?r…ã_-ˆŠ?}»ÌáMïî?ïùˆÞûs?_*:œw/8?I܃K÷?_*:œw/8?ïâÂÝç…?X­J0éÂ}?m=óG4Bå?X­J0éÂ}AGN4FGL J0559.6+3044¿ã™3·ñž@EF%~>ÊÀ:Òn`/ë€À<Gfȋõl@"iôÄb›?ö¯•Ôèû?ÐWN»¤ÜC?Ú¾•Û}À@
¯H<¯³·@0&Ø1¿ïÿ£ž\w¿ïºÔaì""?ïþØ
b?åƒ)ë‹Ôµ¿Ü=½zÊ¿Ûö]"ÛšAGNbcu3FGL J0559.8+304287GB 055627.1+304251?ïهÈá°µ?€ àËÞ?s<|™ÁÐ?€ àËÞ?ï¡¡®?"ÔŸ3tg)?‡—¼W̐?"ÔŸ3tg)?îúæ¡<Ù®?"j<±L˜Ô? Q•íê3"?"j<±L˜Ô?ï¥W-kü†?w´ÌkÏ#?†ª4²¿Nm?w´ÌkÏ#?ïÛ5Aš?qtüDY9?re_&•cÕ?qtüDY9?íf)ÑÏYß?½JôQîV­?´Î±p©J?½JôQîV­?î¥<s‰ö ?UhhÿZÚ?¥¬8Ƅ¯?UhhÿZÚ?î§LäEu'?Ÿc¸Š`ò?¥‹1»¨¦í?Ÿc¸Š`òAGN4FGL J0559.9+6409?ØìøÛc
@2èß?–À:þ¿yýòàÀ<´ZÐ0.œ@f™<ÒnL@¸<½°Ÿ?Ä8âʐž?¢Û=º?á°ê7.j@ž ÀêÁT?ïlËÀ]RÁ?£î˜àJd¿éól|*¿Î7UAPu¿ÝA¡
&¿ç¬?8¥
AGNbcuGB6 J0559+6409?ï<?vöˆ[Nr?aäuAiçƒ?vöˆ[Nr?ïð0–Ãí?`'|³:š¨?_žÒ*6??`'|³:š¨?ïî×ëӒ?h@ò†>L?aã(,n?h@ò†>L?ïèŠw*?GA5úKþ?guðËnMÇ?GA5úKþ?ïî*߸É?hµF¡5<?aåÕ‡‡?hµF¡5<?ïÀlÚHáE?'Ó6€h?ɒőÝt?'Ó6€h?ïí¿Ï@ø÷?q¤{RçB—?b@0Œ,Ñ?q¤{RçB—?ï™BHúÅ®?tsnž+—8?‰¯m° ˆz?tsnž+—8AGN4FGL J0600.3+1244?âã½&ü™Àú¼þ"°À:$™Õ(»áÀ<` SÇþ@#^ÎÚîùr?ø4þ"ÅõB?Á*h‰VUw?ń8Hñ¶f@vQElñ›@–A¬rº2¿ïÿ='—t{¿ï=ÙìD?ïÿtµÍ­?Í'"™2§¿Çh—Ð¹¿ÞqG ¨"AGNbcuNVSS J060015+124344?ï÷w!ìÜ.?QuPí‹ç³?Q¼™º'ô?QuPí‹ç³?ïâ*+š?uHo·FH|?mÕԂ؝Ë?uHo·FH|?ïÕw"?uWžñ?uDpIu‰)?uWžñ?ïËÎñ]®?kˆ8~—?zù–op¹?kˆ8~—?ïâäM
äy?hþ—lèˆ?m³2ô~U?hþ—lèˆ?ïYȵTÏÕ?£z@±ø•e?"ÆéP>›l?£z@±ø•e?îûç•XŸÝ?—uøu_7$? A†§f7?—uøu_7$?ï1Äfï?'K}z÷d?™ßqjNÉ?'K}z÷dAGN4FGL J0600.6-3939?àe'潩À:6¦ڜ™À9Çü6FãêÀ<"š3Œÿ@»3j:±W@nu5¬?»S9¸ÞXe?ÉJ®yûn¡@'ÌÛæED@w‰µËÔT¿±gû;õún¿æJ	¾Å£
¿ë«ð«Ï&¿ëژÒÊ<пí¤Qƒ€R¡¿ïû´áô|>AGNfsrq3FGL J0600.9-3943PKS 0558-396?îòK`óØ!?µIhéHd? ÛIñždñ?µIhéHd?ï^·…î?žf€"Î%?")jÔV?žf€"Î%?î¥Ñ¾×Ÿ?œþFÕB
h?®…¢á~Ñ?œþFÕB
h?ï(ÿ´ðPú?'C/ïú«Û?šà	[¨Ã?'C/ïú«Û?êr\‰ì0?ÀÔt£Z¾?Æ6Û O@?ÀÔt£Z¾?ë•ŸJC×?ÆÖ;¾û†|?驂Öð£?ÆÖ;¾û†|?æڊA¯DH?´ËÒ."²?ÒJë|¡wp?´ËÒ."²?çA<ÛÓzç?·¶Ñœl3?Ñ}†HY
2?·¶Ñœl3AGN4FGL J0601.0+3838¿íՙ̼@›%,à2ÛÀ9{ôörÀ;ýxM·‡@ 1ÊRt?ÿHécˆÖ?³«½ž¹þ?°ўî˜$?úkIÅEïÎ@¯–×óF‰?ïð'Þh¤¿ÖÊ'¿âµŸSí½Þ¿×l=Æþ¿æ·E¡ŸÍe¿ÉJ›Ú'†{AGNbll3FGL J0601.0+3837B2 0557+38?ï÷÷ÿ;ì?C¿àš–Q|?P‰œË?C¿àš–Q|?ïÕµjÊ=?v?¢6\±?u%J«_•Ã?v?¢6\±?ïÛéÝÝI?rädñk?rp%¯g?rädñk?ï+:'~ö‰?m{c盱?š˜­Îi`ë?m{c盱?ïÜÉÆ6?lØ	ªmcE?qô›®Ñ3?lØ	ªmcE?îýÏ+KÞ%?¦Ÿë}]? #
O ¬?¦Ÿë}]?ï¶I'2Á@?…šå@ƒu7?'m¶,'?…šå@ƒu7?ìázè9Ëå? ØQ‹?+?¸ô(½Ã­Z? ØQ‹?+AGN4FGL J0601.1-7035¿ÃhɁ)¥À=¡g‡Î•ûÀ8¹£¥Œ#À;è×Òª\@ñe¸°–@ƒ‡Ä"ÿ¯?£·¦J*ø?½Ò/ãšj@Fº z^k@pM6>«a¿ºŸ»Ç–×ó¿à*Iëœø¿æÖ`)5ƒp¿åЬÀ½ÊÑ¿è·âŸÇÛ÷¿ìT*Ÿ:î>AGNfsrq3FGL J0601.2-7036PKS 0601-70?î{­ìž
?'ú¡
@?¨NE%¢`?'ú¡
@?ïõõ=aèÜ?UÐQukLŒ?T"üõx®?UÐQukLŒ?ïÁ‹ß'î?'ø³£?:^%[û?'ø³£?ïÿe9ž:?Gm	,mU?³W¥vÎ?Gm	,mU?ïø.EÉÉô?Nk¾îO?OFètÉö?Nk¾îO?ïØ|:ä?wb\Ÿëq?sÁâya‰Á?wb\Ÿëq?ï³±GW¤Ï?ˆOºÏà'«?ƒ®6ÍZ0?ˆOºÏà'«?ïý3";—Â?,n ùt±?6cdW©f?,n ùt±AGN4FGL J0601.3-7238?éázÍëI©À=‡·Ïå†À:øz§fÀ<£ñà'Œ7@\\sôC‰@âÃäƾ–?Ä wÚ,0à?§—j•J?åü~ìC@~q'´¿ë[þ*?ïô¤'*è¿ä?ʅʯ¼¿æ«QAç*¿Üá-â'Z0¿Î±k

pAGNbllPMN J0601-7238?ïþײ•$P?4ºäB?""Ø'T–?4ºäB?ïõԌ£€½?XMãL½á3?TVçBnåf?XMãL½á3?ïð鲿8?_Þ®ò?^,šñþ?_Þ®ò?ïûÖI?*k[Ýà_c?@§†wÝYk?*k[Ýà_c?ïýe§,\Þ?/í̀l²?4ÒÆ@½+I?/í̀l²?ïÛðŸBƒ'?tB&+'ôÈ?r°nŒk"?tB&+'ôÈ?ïë#5JuÖ?q~×,<k?dÜÊÙF¢?q~×,<k?ïëÑ9:€§?X¼¡8?d.ƋÅé?X¼¡8AGN4FGL J0601.3+5444¿[`§݊ë@.=Ö[æÀ;7z)'ÉÁÀ<°œÉÏÂK@ Ñ6Œ.!&?ÿ€ì#ª)?ÉÝÂéI/?£Š¾ú?Ùb2z&@gï›û2?Ϲq%\0¿ìÕSïk]F¿¿c"OðÆ¿Û^'¢O¥¿ÛÞ9¿ëížÔkýAGNbcuGB6 J0601+5443?ïþ' ö½?#s5Ø5?&Ýó«Õљ?#s5Ø5?ïñÕ]"?^žì0°?\UDC"‹?^žì0°?ïöϾé+?[Ú¸ƒKÇÒ?R`'­·Y?[Ú¸ƒKÇÒ?ïøY™¥?1€Jnû²?OƜæ%_æ?1€Jnû²?ïþæcæs+?â©û(¥?!™ÄI§ò?â©û(¥?ïŕÛkm"?'	™ƒ)?}5eÆ?'	™ƒ)?ïømMq‰?fµö ?NJÉmæj?fµö ?ïæ7ço\Ò?W¦µí%r?iÈ'侉?W¦µí%rAGN4FGL J0601.4+2320¿Ó-CŸççZ?Íb±%&€À9Q¡/À;?‹!0Ò0@Ò.ϏÐ@#ë¤ÿ(j?Ãðç^HŠ³?ÊÛ9·†¿w?ÿãÿ¹‰#*@©5§¬¬Ç¿é¬¤G¿Òvǝ
"¿êçÓh'1¿èá?(‰â¿ç)\OŒ/N¿ïã²…AGNfsrq3FGL J0601.5+2309MG2 J060149+2324?ïÇÜËG'?}©d'!½V?|šG™˜?}©d'!½V?ï-W@{¼?¢Ø2zÊ£?šUí.,"?¢Ø2zÊ£?î]ŒdÊ&w?™!¬q9]'?ª'9²±–?™!¬q9]'?ïgLÈä?ù÷Zót4?œsfã}­?ù÷Zót4?ë§øI("?ÀªL' s?Á`ºÛ]´?ÀªL' s?çHÁžV¨ê?θs úï?Ñn|ÃR®+?θs úï?å÷f½4?¶ñhfàx•?Ô2…–àà?¶ñhfàx•?æ6Ñ;­'Y?¶µP`=ø÷?Ӓ]ˆ¤ÝM?¶µP`=ø÷AGN4FGL J0601.8-2003?yïÛÀ3Ùä"sÀ::Ó8÷˜RÀ<L•òE,Z@±y]äâ˜@ir)Zl?ÀÏÔ©É?Áª~™8 ?ùA".öŽ@ÞR}T•¿Ï®2M"¿â°FŸ ¿é›H€w^±¿ì|¿8"†?§"Uür'¿ïýïŸ_¬8AGNfsrqPMN J0601-2004?ïþ¡Ÿç*`?$‰áml¨+?%æ PP,?$‰áml¨+?ïö†Ý)fV?SÄI¾‹{ª?RòEZ¼´Þ?SÄI¾‹{ª?ï渃"ŸŠ?lðßLQ?iG|z~¾"?lðßLQ?ïþ'4½™K?fÕ{³'?&ì°V
Ã?fÕ{³'?ïúžÕvG8?Lª<•?E"©í)±¦?Lª<•?ïØ)éÄ?vÙohߺ«?sëÞª?vÙohߺ«?﫛Ëç¹Q?‡#°øõŽ|?…
Ы?‡#°øõŽ|?ïó™'-ìL?Q	{½è?Xͱ¼ä—?Q	{½èAGN4FGL J0602.0+5315¿ïŸ;˜m°Ä@-%åр´À9{ÌÀ7"À<+6
Ä@ÈÏ»i£?þùLVè?®°ÀÁj‡Í?œt2¬Ðƒ?ð'޻♾@'Áƒ¢?æZºÌH¦¿Ô€'ཚ€¿á~•Üär¿Ù5_Þ7v¿ážXæK#¿ÓÂùå3ËßAGNbll3FGL J0602.2+5314GB6 J0601+5315?ïþ¢ýñ\ú?%My¯/ò?%Ð×O¡m?%My¯/ò?ïó£*3|§?[—æÛY8?X¹«Úÿ2'?[—æÛY8?ïø>fÜÇ°?=Î<ÍÒ?OdÒ²çp?=Î<ÍÒ?ïüTå4¢Ÿ?)dVv9|v?=XÕ[ÔÖP?)dVv9|v?ïþz¥V\?ŸB÷F7?(U°ÙcÚ?ŸB÷F7?ïäðîGÏ?"³7¯¬›ù?~-‡y½Ðj?"³7¯¬›ù?ïúìÎR'{?OL«g`#\?DLƪ.—"?OL«g`#\?ïúW‰v-P?9"|T!&?F¡Ùþœ,?9"|T!&AGN4FGL J0602.7-0007?ïáÓ¢)
:À%»Åޜ*À:@x
Ә™À;Ê%o%QÉ@i€0¼áG@S7ë(Ø?Ê$ Eűû?ÃU6hFæC?ô²—,Ê@ÏÁZRÜÇ?æäíU'¿ÒãIüMmò¿éSe¢òð¿àÜ®ÙÄ­¿çãœA¿'ý¿ïÿð`OËðAGNbllPMN J0602-0004?ïð/¥V;?`xø'`â?_¡öáN‰-?`xø'`â?ïÒö¦¼ÿ?"‰á†?v"·Áïs?"‰á†?ï"^*œzŽ?":ôÉô0æ?‹(uR$t?":ôÉô0æ?ïi÷=lO½?nÅìw¦Äi?'Á[
S?nÅìw¦Äi?ï¢'1¯6?!¯^ïþ?+¯½9µB?!¯^ïþ?ï:"ˆã"ä?¤¬âMqà´?˜­nàç'?¤¬âMqà´?ìÊñZ~Y?¬Qs"…V?¹¬u,
5?¬Qs"…V?ëRêô(í?£ù
…j0Í?´Wœ/\J?£ù
…j0ÍAGN4FGL J0602.8-4019¿Ôw"¨qUÀ9÷±ÿÀ9HÙè>B[À;֞-}Í@MË°4z?ü¨zd×ñ?°ûe€Q7ð?º‰Û
¨$¢@
MÆýòÿ@çÖøj¿ïá÷ ³SÕ?ﻹ.׿àƒËÑû	÷¿Õ(šž&q.¿â«¤(hÔÖ¿æ &5AGNbll3FGL J0602.8-4016SUMSS J060251-401845?ïûÜ-טr?@xØNK?¬?@Iƒ˜r?@xØNK?¬?ïçÛὟ³?gïöÖâ)?h$&=?gïöÖâ)?ïÍÁ…à˜ö?zçk#"}t?y<õ–|ÿ?zçk#"}t?ï±D·D?föÒKf+À?ƒ».îë0?föÒKf+À?ïçíåŸ?h5ªÒi(i?hó˜a?h5ªÒi(i?ï–÷y"âd?'³½È}&?ŠB!"x"'?'³½È}&?ï"LZCë?ŒáF2g§?ŠìékÌ©R?ŒáF2g§?îhðN2?—¯ö,‹‡?©v þß5Þ?—¯ö,‹‡AGN4FGL J0602.8+6041¿å†¹'³Kq@1ÒZh+b"À;LN¢ûB+À<›—¸
@çט'Ã>@k¦ý/k(?ÌȆŽàÙ?·sÞt?î'ÿú Ã@p ó•Žr?ïØ+oðRä¿ãDD¾ÂH¿çÂ>hñ["¿ÝÛ«aïÿÿÊPË?ïÿý¡UûŠAGNbcuNVSS J060324+604009?ïò cC?Wډ«¿PØ?Z¿8̼'?Wډ«¿PØ?ïçüËdC?h:¢P"óc?h4\7í7?h:¢P"óc?ï‰~
³-?‰œe$<¸R?»àke(Ï?‰œe$<¸R?ïáRÿ'ƒ?TöMÔf¢?n­qœ|Ü?TöMÔf¢?ïðŠŸ*Ó?ara©c^?^êÁs`Š?ara©c^?ï‹*bÿÿ?'Tnë˜?5gJNô(?'Tnë˜?路‡:œ?ˆ˜7ã£Ö?†Ò9—R ò?ˆ˜7ã£Ö?îï\GÇÅ?e§¨Í.?¡
;"oε?e§¨Í.AGN4FGL J0603.9+2159?íU`U³Ä?¨˜,C;À9g l‡ØÀ;IéÁЈ@‡T>7É@·a*½C?·œ8°J¶¿š€)†G\?ãA® 9[k@	 ˒:*?âÁ?/À¸¿âÀ+i:V=¿ë¦¬ÂkIû¿Ñö0‡ÿ¿ëÄ®…¹èÄ¿˜èíû׸tAGNbcu3FGL J0603.8+21554C +22.12?ï÷Iî5¨.?PÿîÇý9ç?Ql#`u•<?PÿîÇý9ç?ïé¤\HÞÊ?vã6ã_u?f[£è›–?vã6ã_u?ï`¤k7d#?Ú"ûÌwd?"ëršËIŸ?Ú"ûÌwd?ïô70)#Ì?A)¿°N*§?W'ŸJè£?A)¿°N*§?ï©Í®@'?†×D
wÂ?…Œ"b?†×D
wÂ?ïlЕÚl?¢£‹l҈›?'eíMSx?¢£‹l҈›?î|6Ýg?ž»Ü4Ö¨?¨<– w˒?ž»Ü4Ö¨?ᅭR¹œ€?n÷å(n[?€k]Ÿ'?n÷å(n[AGN4FGL J0604.1-4816¿Ö[YÆ"—7À;}Oß;dZÀ:‰øg…JWÀ<|õÎMÖM@!SCÉÙR?ûêï,s%'?¿÷>….?³Íï6¯©?öêºÅ­@ú9lˆ>¿ï°OžMÞZ?ïüÅþ§e_¿ÜÀæå|ǿ܍üb;´a¿ÜÕ9BkàN¿Â¨Xú2ÍAGNbll3FGL J0604.1-48171ES 0602-482?ïÿLN¾!?•'§Ã?}PږÄ?•'§Ã?ïöne?S"J nº?SÃ$&­Ã7?S"J nº?ï÷VÕ
E?@"/ŸC{?QRU¯TVò?@"/ŸC{?ïú	¨]Ø?1>0  Ô"?GÛ¨cØV	?1>0  Ô"?ïþØ»Ëü ?#J¾^¤y?"tDú>ðÛ?#J¾^¤y?ïàKÚ@u?qe(Hª…þ?op³û$c	?qe(Hª…þ?ïõóNì¢*?dl‡R?TaïÁëß?dl‡R?ïìµÍ5?W'"•»f?cýë?4‹?W'"•»fAGN4FGL J0604.5-4851?Ò­Td¹Æ"À;‰¹"¬TÀ;5£ÇeÀ<šó5í"@:^}¹¿)@{\ÚÌiÐ?Åícۜž\?‡5ÖP¯	?ÁÊ'˜˜"@ftá~_¬?ïõœdO4ñ¿å›	Ü!Ôf¿éë‡ç`Í¿ÝÖÚhµÌ¿ês€€C¿»4.A2³AGNbcu3FGL J0604.7-4849SUMSS J060433-484947?ïügyáÃT?6äÌEd,?<Ä1ó.…?6äÌEd,?ïöÉ=©·R?SýSéé=ž?Rm"( ]…?SýSéé=ž?ïè"Ò°;?eÄ\äN?gl-M³v?eÄ\äN?ïü'¤¹™?!ÈO)Y?;ë| ÁEš?!ÈO)Y?ïñ·r[?` :
g#ª?\'*±º?` :
g#ª?ïݼ)«?s¨¿äË^?qr÷"^†?s¨¿äË^?ïáÆ	ݛ?sVaHâÍ`?n9ö°ÈÍ ?sVaHâÍ`?ïîn%U,¶?QMëcšgø?a'Ú"ÕÊU?QMëcšgøAGN4FGL J0604.8+4411?ß/썲[@%Èù±1eÔÀ:ecãÔPÀ<Ȓ«hÏ@:"çÛÇ@oê#èù?Ã×ã–½Ç ?«M-5?åŠgAؒ~@˜Õl²?Ûú"•üV'¿æ»`(^ÃÛ¿âèìô,¿ê§Š$Ô¿æ²^âc¿ðAGNbcuS4 0600+44?ïýoíMË»?'up~‹nH?4€"²?`?'up~‹nH?ïïJ{4?b 
Ÿ[Ɂ?`êµXÐpW?b 
Ÿ[Ɂ?ïæžKžÓ¯?sŸ]´HŠ?ia´ç¼?sŸ]´HŠ?ïñwù®#·?@ǖX7¡?]QAó?@ǖX7¡?ïûbÚs\?@È0áÌ"?AŠtóã]?@È0áÌ"?ïN,ïÞ[?"Îúüuô?‹ìtÎW=3?"Îúüuô?ïÞÏ÷Æî?u‰TÌ»Òû?pô[™?u‰TÌ»Òû?ï®'±'ˆc?p	à"]r?"v¯–¥X?p	à"]rAGN4FGL J0604.9-0000?ï U'¤´«À$§ñQçSÀ9Ö¡Š(ãNÀ;ëŸ+©Ñö@ `|°Ä®?þŤðñ5?ÁÇÓ(["Ð?Àöh½ÕG@Õ%`â™?úé!>"l?ȏËåq3t¿ãP´î‰µ÷¿ÛžgŸ —$¿àÕß?Á#¿ÍÎùÁ¢w¿ïÿú Âî'AGNbcu3FGL J0605.0-0000GB6 J0604+0000?ï÷jR.K?F¹ãÈù‡E?Q+[Y2Bh?F¹ãÈù‡E?ïÁqc^bü?€cM*H߈?GN=²R?€cM*H߈?ï´éר%¬?óÿTW?'ÅŠ(a?óÿTW?ï]ºÿ¬e?u<'lj¨?"H X)n?u<'lj¨?ïƝÅ<$?ytîd@|?|ô13âR?ytîd@|?î™Û…9x?±ŠÞV<A?¦bG­Dš"?±ŠÞV<A?î¥8¡\0­?›Ý[þ='?¥¬uê<õ)?›Ý[þ='?뷚Ï,V(?§ŽðqN?Á!"ÃN§a?§ŽðqNAGN4FGL J0606.5-4730¿ìßÄaøÀ:ò|ᛑÀ:iƒ¾f½À<~)gØVn@¹_÷·\"?þSó?ÀgX>Zƒ¯?Ä5â:[€@Jb#ᆘ@ÿ8¯ÉÝ¿Ê~ÆÀï?ï†va[9¸¿ØBµ<u¯¿ÛlÛ z3x¿ã'ÿýPοç¸u'8)AGNbcu3FGL J0606.4-4729RX J060635.9-473001?ïÔ¾¿ž?®¦Qé|'?u  GShÂ?®¦Qé|'?ïó¸³T¢?V0¢ia?XŽ˜Ñ
º?V0¢ia?ïñ…RS£°?WN¿•©i?\õ[@À ?WN¿•©i?ïß´¯ZÝ,?R°ÊÑ©Ö?p%¨7Äuç?R°ÊÑ©Ö?ï÷«#@=?K½š®Nv?P©¹a´õ›?K½š®Nv?ïÏ«Õ9
–?Š&àð•\?x*I]­?Š&àð•\?ïàL€ƒ•n?r€£|
?o³kìre?r€£|
?ï>•Ö°??wöZ8%xo?‹ðZ|•€D?wöZ8%xoAGN4FGL J0606.9+4402?瘝wÁúÙ@&SZBkµ[À;ˆ²køvŸÀ<¯
¾Ÿã`@"vJâ§T˜?àÖ`ÿõE?âÌ|ý?ïÿÿ&¦³@™xâií@žÔ2FÏ¿ì?2_Μ±?Ûìû@}ž'¿æïa¢1n¿Æ`¯Z9²?¿ÒČ¿ïÿ̞©£ÓAGNbcuCRATES J060650+440144?ïÌ%s"0Û?™º'#r…_?yíFªb¥?™º'#r…_?ïë6²n§¨?lhF
˜¤?dÉM»óJ?lhF
˜¤?Îc$è?Ÿ*sõYٜ?§ö"=Mt?Ÿ*sõYٜ?ïõ.ØÛxâ?Kò9àÅùÿ?U¢Mó×ìN?Kò9àÅùÿ?ï븙JO–?tïCýZ?dGfÄβE?tïCýZ?ï{Gñ¨›·?˜šlàûn?—ÑËÁ?˜šlàûn?ï Émê
Ã?—4´Ò*?›æÒGæ¥?—4´Ò*?ïëݧÄ?hæ	ÒAKê?d÷"aÚà"?hæ	ÒAKêAGN4FGL J0607.2-2518?æêÐN^ïÀ4mÙ ð¥ðÀ:ñe9?¼®À<­¢pØ°0@ Iý?üÿ¥·µ
"?ÌNÖý¨7?ÒûG¿1X¾@*3<m@î" ÞÇÌ¿ïÿÝÑô?ïòÑ®³Ý¿Ì°B'—É‹¿Ô§â݅W¿è…ÀsοÆx øóò+AGNbll1RXS J060714.2-251855?ïüŽœ÷ƒ@?2#ó	M¯ú?;‹¢tÙ]?2#ó	M¯ú?ïíÚH,áØ?af/kM?b%·»ÀÐ]?af/kM?ï±D@Kʄ?']Õ2øÖæ?ƒ®ïàVÑ ?']Õ2øÖæ?ïÃk=vê(?_<Ã{•/?~JaEêÃÌ?_<Ã{•/?ïùT䢛:?HݼªB?J¬ldXÇ?HݼªB?ï¬å)®ü?‹‡y»À¦r?"ƵºA?‹‡y»À¦r?ïhAÐYõ?'±·3»³?'÷Åöy+?'±·3»³?îز» ÷Ô?ŽMwvúå?¢tÔE›¾?ŽMwvúåAGN4FGL J0607.4+4739¿ä"oLi@)»ZBkµ[À8KÅPÉÀ;‰†¶hz@hÛ!yL?ÿ묋å?Ÿžöaù?²î˜àJd@Éé^ÓÊî@€9Küï?ä·¬ÿýѧ¿Þ­€×*ô ¿ß–7D9ë´¿Þ9p¤'Öµ¿ä,™¦5¿æ%¢HZãAGNbll3FGL J0607.4+4739TXS 0603+476?ïûÕZÝ=«?8ñGžyôJ?@ª"sò[ç?8ñGžyôJ?ïãôS¤lÜ?ugÏ37ǎ?l¬ST¿?ugÏ37ǎ?ïæÇr£i/?q/"@?i8F™QS?q/"@?ïãé¼$g?RõtÙù÷?l÷F›Ib?RõtÙù÷?ïý2°"ê]?0Xi´]Äô?6j~j;w˜?0Xi´]Äô?ïhDì‡ìã?œ?Pýè[p?'÷brqÿ¥?œ?Pýè[p?ïÝ—†Ím?€Cu6°?q{´MÇUŒ?€Cu6°?ïž2$ëFà?rPƒíâ#}?ˆsvÁ¾«ì?rPƒíâ#}AGN4FGL J0608.0+6721¿å/"ƒÁQU@4ßH!ÄvÀ:É¥Ð߁À<rÁÄN¯@Ô®rC¿G@e²€fÃ?·_ïÕ?¶O•¿ol?ýŒð=ë@‹ëëv@?ïþ¸*¥¿åڀ¶–*¿æšmÔﱿç
ýQúÊ¿éOt¢>XÖ¿ïüßÿÚkFAGNfsrqS4 0602+67?ïýÅ ˆ¡$?$Q-mžš?1Òû¹ÝgÛ?$Q-mžš?ïóεÉê´?Z×(]{¸?Xb" d§³?Z×(]{¸?ïêX"xG\?RžGríÍ?e§ÝÂÑë×?RžGríÍ?ïúë»ûCX?0E)e§"™?DQÂQã2?0E)e§"™?ïýl­8™?.sl¬¢"?7ä˜Ä	ÓÒ?.sl¬¢"?ïÂP™ÂÖ¡?'xZi‹ê?~׳X"?'xZi‹ê?ïÌ~ª™µã?{Rw)?‡?yÀª¡÷£?{Rw)?‡?ïòd‰A‡µ?HHì#oo?[6í@wvÔ?HHì#ooAGN4FGL J0608.0-0835¿áX¢X…À+-{cM­À8z!ÛòÚÀ;gUá³äž@Vä£-@ÝÛ?VW?§ åþ¢û?²#ì€ÏÚ@M­àx{<@­þ/Eh¿É]úºpª¿áé1â¦'ò¿å¬¬›ÔÝ=¿år|õ$®¿ëÏY¿Žö¨¿ã‡%Ž/AGNfsrq3FGL J0608.0-0835PKS 0605-08?ïøÕQ*¿ò?rCê¡Þ/?Lª»uoº?rCê¡Þ/?ïöŸ;š
?SÅg´nµ?RÁˆP:é?SÅg´nµ?ïµã¶7"ñ?ƒþ"/¬ÍG?'‡rç/Ò?ƒþ"/¬ÍG?ïþÿíêw?¡&!Q+Õ? ©V?¡&!Q+Õ?ïû¢ïiëè?<{¦"5b?AtB@¬©
?<{¦"5b?ïÔ£+¤Ú§?'g'A8Š°?u®jOîĈ?'g'A8Š°?ïž&Ä?†¾èÓ»?ˆ¶íšð?†¾èÓ»?ïýŽ›¹¯d?-ÿ(¯k¦ä?3‹!‰1½?-ÿ(¯k¦äAGN4FGL J0608.1-6028?è:ñ"½aÀ<¡ð†nDÀ:+>WS£ìÀ<
¢"ú¦$@Þ)=Ðñ@T™Â´E?ÅÆæXäóŠ?ÇU¸a°Ê@¥á¦x¥@Ô&Z²©
?àî姏&¿æf¬![š[¿éq+¼FlÌ¿éê šª;¿ïÿøþÙå9?äãÀEçAGNfsrqPKS 0607-605?ï÷«|xª?ot#nî»?QÞ¨€]ü"?ot#nî»?ïö´µ?UIRÙ¢I?SÙÞèŠä?UIRÙ¢I?ïËhÞx­?q`¿/m½[?zKðuöµª?q`¿/m½[?ïùæÐý+?4*š,Î1\?Hd¾ÛÜ¿?4*š,Î1\?ïñ¿^éß?`ü­®X&_?\B¥4	?`ü­®X&_?ïÓõӁFç?MÈ6šXÍ?v@xG?MÈ6šXÍ?ï 6þÈ?"S­½m'Y?›ù=ùGŋ?"S­½m'Y?ïÈð˜?7µ?k×—LgÙ?{‡³ãÓÁ·?k×—LgÙAGN4FGL J0608.1-1521¿ã~GÐñlÀ0aóFí$À9²L‡À;ãIâ¢!@ª<ANÔÏ@aÏBÈÒl?­Q4¿¿	?µåê**ËÜ?ÿG±õ°ñ¥@ô÷ή#i¿ÐFŸ ¿â-¸À%t"¿é£€}"Ô‰¿æ5v•ˆ"¿é"|žâê¿ïÇõAàõúAGNfsrq3FGL J0608.1-1522PMN J0608-1520?ïþ¦ð¼Ž?"éBf$˜?/ՔÝ#G?"éBf$˜?ï÷IS—=?Qbèˆb59?QmYÀf?Qbèˆb59?ïÝCßA³B?pl2Š60?q^gen·?pl2Š60?ïÿŸã4Ã+>ûX'ÀM~"?@‰?8r>ûX'ÀM~"?ïýzPlî°?.CDw;Â?4-{pž¹?.CDw;Â?ïܝ¥Ë^Á?·wž<s?q±-@Ûi?·wž<s?êHˆ°?ˆµ§¼6µ?ˆ›Å{œCó?ˆµ§¼6µ?ïÿ>NšAà?o "©x?6$3§f£?o "©xAGN4FGL J0608.9-5456?éo-&Æ`À;Þâ¨dªÀ9·CsóãÀ<^ÄÞÁÁ×@Û]ˆœFG@""³º­?¶æPV"œ?Ø*ƒ·/,@ö"aKts@[ûÎíäJ¿â F\㕿ãíÝÞÂî}¿è\…qÄhz¿ëZ}ú×¢¿íÓø:8á¿ðAGNbcuPKS 0607-549?ïúЕ!é?E˳÷ƒ¤¤?D½«ÀËæÈ?E˳÷ƒ¤¤?ï÷3j¾?Rgæ,¤4?Q癯т×?Rgæ,¤4?ïÐËßÎ?t_Âv¨?wôÙäF?t_Âv¨?ïûˆfb×Þ?.ðžXžx?AÞf1Ò:?.ðžXžx?ïû»a·ÍY?;n^éoB?AysSÂ?;n^éoB?ï׶'œ?ƒï­Å(?t$ö#ô)?ƒï­Å(?ïqÀZ´½ž?‹Ý =ߔ?'Çô§°~P?‹Ý =ߔ?ïê(€î'?Y‰8®^V?e×û³Kè¨?Y‰8®^VAGN4FGL J0609.0-2219¿íTÊM§¹ÔÀ2ñåÀ¹™À:ãêÀӚFÀ<x
œ;4‰@õ¨ä_@'‹vÁ?Ò:og–è?Õ£(c¡e@°ÄXŠÑ@	ªçŸ¶ê?äEôî¿äb¼ÃjM|¿ßM<+¬¿á¡4x­'¿êƄ^I¿ß·$¥Ñ¶AGNfsrqPKS 0606-223?ïôÐK~Ðã?fÿ' ï¸?V_iÛ3?fÿ' ï¸?ïôZžÑÞ?VäÚD5K?WJÃÁ`?VäÚD5K?þ~[â?…a™…ÊE?ŸÀn'w?…a™…ÊE?ïìûyf&?ByËąÛO?c† ¹5¦?ByËąÛO?ï÷]¦õ‰?PgAš¹†?QEÀùŒÍÉ?PgAš¹†?ïÕ/ÀÉ ?x'+'wµÈ?uhzvð?x'+'wµÈ?ï=Œ$]yÐ?'B2ÌÓO??˜N{{/ýó?'B2ÌÓO??ïªÈOÐ?nŒ<ˆ¢H?…MÿžM‹ä?nŒ<ˆ¢HAGN4FGL J0609.2-0247¿ïʋDþHÀ%Q|=h@[À9‰PÉSœÀ;Êrß­*@ 7QŒºŽ?úºܓn?¸õÜ»'M?LJeºnü7@«3¥Cò@˜¡˜–N¿ïÿC*!<?ïýûþé‹¿¦`ʛK¿ÔŽUëæοÚbX"üS£¿è'kr>á½AGNbll3FGL J0609.4-0248NVSS J060915-024754?ï2±·-åR?—ìì÷ã©?™©ÉëÐ?—ìì÷ã©?ï-Ïޜzl?£n£ÀœºL?šF'IHˆ?£n£ÀœºL?î¦1ý©?š?»I9ã?¥Ÿ{(Wr?š?»I9ã?îÞøkê'c?'ÍkÍf?¢yC§Ë?'ÍkÍf?êGMÀ?ÀmOkÌ?ÆãÒ˜ÿˆ?ÀmOkÌ?뛫:3‹%?ƀȧÏv?Á'S1Ój?ƀȧÏv?êéͺ™ª?¯]ºTÖð2?ÄXÉ™U?¯]ºTÖð2?êö²5?® :½›?ǔ'÷7-?® :½›AGN4FGL J0609.5+1402?ãÊ­úí$À&ü›ÇqCÀ9¼ˆ\ZsêÀ;P°Å/Iš@×r'¦
@.—ÂÿÄq?Ëaë¼?ÍÍړßÆ@yŠ˜?ûptgÊ?ïkcÉ€?Ñ´GDãù¿çt÷Ãñ[ø¿éxv¾ù$š¿ãºàŽµ:¿ï÷šÁ6ì{AGNbcuNVSS J060922+140744?ïãLۓå?f¦çPËò?l³è#C?f¦çPËò?íyEf;ž<?³ĝ!(?´5ÔÌÙ3¤?³ĝ!(?îøT?ÃXá–Ô? z¾Ÿ"õ—?ÃXá–Ô?ìäŽ#]–ù?–­
¢‹Ô·?¸ÛŽã[z<?–­
¢‹Ô·?ï< pý‡ï?—}ëÆâ?˜{ñèæ?—}ëÆâ?Û3ÎÛè?ÒI¥Í¦ÞÉ?âæ'õ?ÒI¥Í¦ÞÉ?çAM˜?µõdgÕõ?Ñ}çãdÏõ?µõdgÕõ?ٙú•»q8?¸#u}•?ã3µ"Gd?¸#u}•MIXED4FGL J0610.1-1848?êÓzóùÀ1Sü¹#¢œÀ9Ü36ÌEÀ<(!à$˜f@Ž±¥ÿÙj@SI€C‡?ºbe¥Ì,ê?¸NPº*?ýãGG½-ó@
âmúy-¿ïΣ Öå*?ìû‡_Û1ê¿äßzïŠf÷¿åu{aöD¿å©ø¡çÆοïÿ"ÞïAGNbll2FGL J0609.6-1847PMN J0610-1847?ïþNDåö?˜dè£P?+¯'VMÚ?˜dè£P?ïôXFèò?X)t¤Ç?WOqá#…é?X)t¤Ç?ïàáûÞÎ?q‹x¯ï:n?oâbÂ4?q‹x¯ï:n?ïñvFЖR?C™h†t?]rφŠ¦?C™h†t?ïü:QpÇ$?9®Kæ×1ò?>-s8¸1U?9®Kæ×1ò?ïÖ$Uä|Ü?[)öaYV?tíÕ"M?[)öaYV?ï'ò¿gl?â©zY¯Á?CPBÕÀü?â©zY¯Á?ï¿aC*»Ú?q™ 'Ž¿í?€'¯.qр?q™ 'Ž¿íAGN4FGL J0610.7+1656?¬{ïñ‡D¿ð%Q(ÀBÀ9&ÞßôǾÀ:ù^³ê}¸@ÀØNá£@6þ.n¨T?ÏiE~d^ú?àó°0´Ó²@ê¦ÒgA?ôWTБӿ̼°à]"p¿áO^AÔ¶¦¿ê¨ªxäî,¿ë6Èéé¿ð?èÞ¸AÐYõAGNbcuMG2 J061020+1701?à[^Ö$9p?ÓG˜?Á?ßIBS· ?ÓG˜?Á?ÂO˜8ñc/?¾økÐÍQF?ëlñç4?¾økÐÍQF?åо@íÛæ?±Ø)»#ýÂ?Ô^ƒ~$H4?±Ø)»#ýÂ?Â[É£ç?.?§¹È¬4Y'?ëi
—05?§¹È¬4Y'?Ôï¿Úººë?Ó¢…@q4K?åˆ ¢¢Š?Ó¢…@q4K?tuš\Ô?"E¿D&Š(?ï'.+j­?"E¿D&Š(?ÖÎ|›˜2¢?¸&‰Ua'è?ä˜Á²3æ¯?¸&‰Ua'è?[àH2©_‡?Q芧ëV?ïòÜçà?Q芧ëVMIXED4FGL J0610.9-6054?qgTÀ<TÔÜeÇÀ:Vªñ°±äÀ<%ÚV"K"@Ës0yE@|#ßÙ?ÂMò?¿1ãÁŸ¶Ù?ø¿}Xñ3@
5¨µv	¿æ5(¡ù¤¿à	+ÝÔ\
¿è'Bbûù¿èG"žy_¿å#—´½¿ïÿ¼C͈AGNfsrq3FGL J0611.1-6100PKS 0609-609?ïþ˜õáw? 	ôÂôU?&¾:.˜M? 	ôÂôU?ïö0ÈÂ"?S®×qÖ
?Sžnµ~HN?S®×qÖ
?ïëG˜8¾?lîU±€÷§?d¸âIŠ²Q?lîU±€÷§?ïú…9^W?/֗v]»+?EëªÙâY?/֗v]»+?ïþ2eácæ?&6ҹǰ?,Ù fºku?&6ҹǰ?ïÚú@•-?Bß{?r'õbu¢?Bß{?ï»èÍB?ƒ± ~¤ç?øø"ÍŽ?ƒ± ~¤ç?ïÒâ"Îó\?iãÓƆw¬?vŽµ¸Ò¥š?iãÓƆw¬AGN4FGL J0611.1+4325?ïëÛäJu@'"ãq*À:ù»9À<Bˆ4ˆ@ «*èáÖI?û¬½³TUÃ?ÀA+‡‹O?À`Ò}»ÂŽ@*§Xžý‡@÷˜OŽ?ï9Õÿ{u¿㒰qLsv¿â}§Ë‹"-¿ÍzwëI¿ßõu|Y¿Û­A—$AGNbcu3FGL J0611.2+43237C 0607+4324?ïú~3À)"?:@.<"?F1ôŠÛâ?:@.<"?ïÚäØY¯?uñu–ä—G?rò±_ÌU?uñu–ä—G?ïã( §ã?sÆabp?l€Ø?sÆabp?ï•&ž-Î?f">ª@v?Š¶XcÀy?f">ª@v?ï×´ûß	?oßÿš­?t%òÍ«V?oßÿš­?ï9Í0[#?›û@À?˜ÏÆV"ÿ«?›û@À?ï™Ñ.ӟq?‹q²[¹ì?‰‹´Q÷[¦?‹q²[¹ì?î.÷ÕAÄ?Îìˆ?­ð€.Ä?ÎìˆAGN4FGL J0611.6-2712?³*Ù"­À42®žä\6À:TWLíï\À<~vQ•ôÉ@®Š5x‡Ñ@HÜè£Ã?ÂE³ÆkŠ?½DÙMäa?÷Và·e\@¨AƒMÓ?ïÿÂÝ_¿åeƒGG½.¿å»;ÀJˆd¿äꨠÀ€¿ð?ï©·¸iAGNbcuPMN J0611-2709?ïþ`¹åO·?2ŒÔ•?)ô^`Ê¿Ì?2ŒÔ•?ï÷N·âɨ?RH=@¼Ì?Qbq°?RH=@¼Ì?ï¸æ0ԑÆ?"igù<°?Æs¾Ôì ?"igù<°?ïÿ,î¿?	¶^U›?b='OÇÕ?	¶^U›?ïÿê|Ô?:GŒ¶l?Åqƒûù?:GŒ¶l?ïÝÂâNzs?}‹¯½œª?qŽÌd.Â?}‹¯½œª?ï¸zÚ´
†?‰"éæ¿æU?áIcz¾'?‰"éæ¿æU?ïý†,n6Ù?'XŒX‹ÉD?3Λ‹æ˜p?'XŒX‹ÉDAGN4FGL J0611.6+2803?Ä´o
YD@Ð]{ZÀ9ïËñqÈÀ;Öè`·Ñ@õÒö\")@æuš¶Ð?čaûÁ?ƨºžÌßA@ÓrSÍÝ@ʺˆýj$¿à4³eó?Ö÷PÄh¥0¿ÚÞŝ®|*¿ä2>@­o¿è¬QéØ¿åd¹½üOqAGNbll3FGL J0611.7+2759GB6 J0611+2803?ïôÌmP?Sßw#>ö?Vgó}¿_-?Sßw#>ö?ïÙ};âPº?{høÕOæe?sAb&võ?{høÕOæe?ïÏèÓ
 ?wªÛs¡<ò?x–—̱ê?wªÛs¡<ò?�°ì
?^y…ÅF²?€»Ï¥uj?^y…ÅF²?ït¥:Ùè?"uQ"0ôÌ?'kX¨2š¤?"uQ"0ôÌ?îåͱ¢>?ª(B±æ£?¡£.ÕÁÃ"?ª(B±æ£?îhd6¬?¡žcäñ?©y¼œpÀ?¡žcäñ?î¹ø#4.þ?ŠÂ­)½jd?¤`}ÏPÅ?ŠÂ­)½jdAGN4FGL J0612.5-3138?îÍ4¸æ³JÀ5Œ
9>åïÀ9覨uÕoÀ<5Ûèɂ•@¸ïË)Š@îòžîm1?¶1Õ i"(?­õ}FLÒ?ñÒ±HL@³×1)Þ?Ӭȵæ×:¿äayÝf¢÷¿çéµ²¿èfu 3Ä¿æTg–NÝ¿Ø­>2­AGNfsrqPKS 0610-316?ïþ軕ÂÊ?(ŽV ©¦?!tDÄpBY?(ŽV ©¦?ï÷$£'/²?QáÚóMŒr?Q¶¹%Ø,)?QáÚóMŒr?ïóWô†z?cMäóÜé?YQõõöËÔ?cMäóÜé?ïü­ëé¦*?%Ò=oº1œ?:ž¯"ìr?%Ò=oº1œ?ïþ}!z	?©§z¼zÜ?&ø+‡>F?©§z¼zÜ?ïÜ4V?|ån("‡ÿ?qñòÆèy?|ån("‡ÿ?ïðêžnëp?có|UèG-?^*Ãd!ŸX?có|UèG-?ïòµJ?LJBl¹z?[Εâqe?LJBl¹zAGN4FGL J0612.5-3934¿³˜äÞì}ûÀ7ùrÿÑÜ×À:ÒȏPj|À<a3œå~t@蜞¶@M¹â}q?Ô%j­¥j?Ã÷‹<^«?ìJtÎ6/@ØCÊZ+Æ¿ã<~֟´f¿èâzžµÍ¿æ+@àðÆ&¿àó"aÌMÌ¿ïÿÃF1=¿åœúÂSw AGNbcuPMN J0612-3939?ïý]ܲ¦Ž?.Lî÷º?5–g5?.Lî÷º?ïö!4?VH9ØþYC?Sù½QèÅ?VH9ØþYC?ïÞ1çp?qºõÃ?pþç"wÇâ?qºõÃ?ïûm#Cý?*nxâ§?CŠLZbˆ#?*nxâ§?ïþ†"™]	?'I šØ?'×Y"?'I šØ?ïÞñ#]?qÇV·óŽ?p‡n=‡4f?qÇV·óŽ?ïÀRv¼Ü?ƒªx¦½>?Öú4#r?ƒªx¦½>?ïçÿÿ»GÐ?X"qôßox?h=Ø÷ª?X"qôßoxAGN4FGL J0612.8+4122¿âWÉ]#@%ÚËB‰ŒÀ7ïßlÁÕÀ;YKHÓ®h@wáú†n?ýQýýûC?" ç^Ñû?»Ù¥ß^[@ ¶ñýÞ½@¤e¹˜<¢¿¾+"˜†I0¿Ó™ä'¡¿Üýüdêæ=¿Þä[^Ëg¿ä	ó‡K¹¿æ°T%òAGNbll3FGL J0612.8+4122B3 0609+413?ï³¹«æUè?š¼ºò4u?ƒ"÷¤3ø?š¼ºò4u?ë'
©½?ÄcçâcB?ù÷Õ[‰
?ÄcçâcB?îä^~2?£Ÿ	û>k?¯¾»ÏêÞ?£Ÿ	û>k?î|ðà—Ø?—±–°1ì?¨0ñó†ƒ?—±–°1ì?ï£ôÐ,Ü?Šq@Óèq"?‡߅ü?Šq@Óèq"?Õ¸_έޱ?Ð搤
Í?å#Щ§?Ð搤
Í?ïUScKÌ)?"ª«î8Šê?•U"'_ñ?"ª«î8Šê?äì'ÝŠ?¹	½v¡$±?Ö'ÖÜxÄë?¹	½v¡$±MIXED4FGL J0614.8+6136¿Û
(l¥÷@3Ùb¶®À: èj¸¿À<l³â;ë@35í!Öê@ž7€ŸÍ?Ë<b[ê·n?ÎWÜö:¯S?ûUÕ¤â¢ø@
8Xöh?ïˆ;¾/á¿Úf2CÊF¿éƒ<€8õj¿ç)L?Í¿ä됧'i¿å"ߨò}AGNbcuGB6 J0614+6139?ïø ôþÑ?p"7Ýp"?O|.{	BY?p"7Ýp"?ïôíö=4?XŸ<ž|dx?Wø$"XÌ?XŸ<ž|dx?ﺵÁ¾ý?|-/YÏ?R¼évä?|-/YÏ?ïõdˆÀ®[?8àÔVÕ*1?U6îñYÇ?8àÔVÕ*1?ï÷¾ƒ«=?SSoãôE?QÀƒ'äò?SSoãôE?ï¿t>b³¡?‡(¨A‡q¿?€"ðuÁs¸?‡(¨A‡q¿?îìM·ö?™ñä…çeH?¡;$"žÔ¥?™ñä…çeH?ïÁ
2¼|?i?ŒÆÄs?y1lÑ
ö?i?ŒÆÄsAGN4FGL J0614.9+2426?Ìԗ±âæ•@§TßÔÀ:‡²Â_‹À;ó
8h&Z@´•‰¿‡?û´Õ)' ?Ø쒅(Ht?怸!D@X`~Åؽ?þ®ÓdìhÉ¿ïü0g¦ØF?ïüÕÞÄF?™óMa[¿Ö'×ÞxÆ»¿ìÛU%ÌB¿ïýCŠUAGNbcuGB6 J0614+2426?ï)#<"Ï?ŸyðìB²"?šÞ›ëB)?ŸyðìB²"?ì<xaL?ÀÚHWÔõˆ?¾çô<õ¡?ÀÚHWÔõˆ?롤;D?§+ƒh§J?¹yoï?§+ƒh§J?ê`þ†û?£éO+º­‹?Æ°ä?£éO+º­‹?ìQ4[Yöt?ºð *q1Š?½v]%0L_?ºð *q1Š?ã_kªñj?ÑàxN#??ÙA(«è-?ÑàxN#??æ³ÜRž)ï?¶Â†Û
"?ҘGZì#?¶Â†Û
"?à2_՗e|?¼Ñéä'"?ߛ@TÑ5	?¼Ñéä'"AGN4FGL J0615.3-3117?íQ®žìó;À4ÛaE•5‡À:Uôÿý²À<hÏ(ǟf@ú¹žßZ@Ò[YÂéõ?½r¬Dìï?¦¦˜ZªEŽ?ç/œÛmy€@Á–vú]T?ïþ?üšE¿æ¡³^f½¤¿ã&Àþb¿áSÅDBO0¿ãÖàµwF¿Ýš_ý–™4AGNbll3FGL J0615.4-3116PKS 0613-312?ïþ¾Ø °?ºñQ/+×?$|?î%P?ºñQ/+×?ïöV°)¶?UøFù½´j?SR n¥?UøFù½´j?ïöðŒ<a?c–FÖ暖?Rç'uݝ?c–FÖ暖?ïúÈ'÷jÛ?+Ý28cnŠ?Dß`Èè	*?+Ý28cnŠ?ïþ¡ÆŽÅ*? NÓ-ÍÐ?%㕼¡*—? NÓ-ÍÐ?ïÞ+p€ð?u>L­‰æË?pêHýø?u>L­‰æË?ïùªjđa?SkÈG!g²?IVU$´:;?SkÈG!g²?ïñ^>ϞŽ?G—Ñ.Õõ"?]C'óÙ?G—Ñ.Õõ"AGN4FGL J0616.1-1732?Ø0eäÀ/j;Ýü À;~ì\µ½À< Òc傦@!÷ŽsuÃ|?öښéœ?åö\å®›?Ù¨Ã"ð?÷†D·%?þўEzÞn¿ïþ'!€-b?ïôJõǗÚ?Ñú±AV¥¿Ø2ÒûÄ¿ÛÓmE'ÒW¿Ü  0÷ïAGNbll1RXS J061609.5-173313?ïû­ät?@Û»^ÿÐ?AHn¿xÜ:?@Û»^ÿÐ?ïíÒØnZj?`§ŠlƒÍ‡?b-'Ë_<?`§ŠlƒÍ‡?ï½µBË	\?s²~nç˜?€'¯OýY?s²~nç˜?ïÕ»!Ãc?^F9k?u"o*­3?^F9k?ïû
€­J¸?@ÓjÑÕ?CÉý)ØáÄ?@ÓjÑÕ?ïÁ Ú^8x?Œ/L_.X?/'Öc#é?Œ/L_.X?ïÑÙ@ùom?|©¤Õ©Â?w_ƒHIp?|©¤Õ©Â?ï‡N:B–?€t&ÌR=Œ?Ž,qrêö\?€t&ÌR=ŒAGN4FGL J0616.7-1049?ÛeÑ£À)"Í[h£À:N.a<[À;¢ûú·Á£@G˯ÁN>@ãÖáù"¼?ÐÄR1ž‰?Ù¦žD¤Ù@ñ©áyñ@—rÄÔ?ïÿéà
v¿è@‡å</[¿ìcMâáâ¿èá}ÿ	_û¿ïÿÿ" 5•?ïù*ù¨ÍêAGNbcuPMN J0616-1040?ï^"°!y?¥ƒ#¸M?"-ÁdÊì?¥ƒ#¸M?ï#6üÉó1?§T'•wã?›™ kéÐ?§T'•wã?í…i7•Ý;?ž í2äQû?³Ô¶Eä#?ž í2äQû?ï*DÍ'?ƒ}
¿¶?œ·bî'â?ƒ}
¿¶?î`dŽõÑ©?¯üÞøÉTó?©ù·¢ås?¯üÞøÉTó?äF<kÚÞL?ÑÈïúñš¯?×s‡(JCh?ÑÈïúñš¯?æj.`KÖS?´Í‡'?Ó+£?hSY?´Í‡'?ã=ü£»AÆ?ÀIŽ"WæF?ل¸‰|t?ÀIŽ"WæFAGN4FGL J0616.9+4340?íuôØüÓG@)<ù;À oÀ;ÚÂXՄÀ<À­°i@"—¤}£Cç?ù¼'«A?Ø	zg¥*Ç?¼O ÒÀ?éÙ? ý&?÷Š¿Ì‰0¿ä¿@OÁß?ï«ù4㍿ٸ)|¦Ù¿Ý&c–þ4?"™húÈç¿ÜºÉ?$AGNbcuGB6 J0617+4340?ïþsãI}?»Ï`S¬Þ?(ÁÈ#±?»Ï`S¬Þ?ïàÞfŸ"¦?|
X"Õã^?o!™…ˆ!Å?|
X"Õã^?ïêU7®±È?`™$núÂ?eªÈy)¯J?`™$núÂ?ïéÑQ/·B?UqÄ1€})?f.®ÛG~b?UqÄ1€})?ïþJEÿc?+,73[?+[²ùY×ñ?+,73[?ïV6ª®aI?¤æÄYÄi?•9*¯[@Ñ?¤æÄYÄi?ïåLÆF?päå!IR7?jb³^Õ¹?päå!IR7?ï~Ok£=?ˆs‰JÓ1?6'}d?ˆs‰JÓ1AGN4FGL J0617.2+5701?î*
ÍäNõ@2ëáe
FÀ9I"žˆÀ<(ØåßÃJ@‹AÑ܁ @a´5&Rz?¦DpÈ??§_™m¤É#@"'Æ@
Ð-µý­¿Ñ£ˆ{>1¿áZºÌH¦¿âA¬=
LŠ¿Ü"ëø>ø¿åø| µ¿ã^'/éAGNbll3FGL J0617.2+570187GB 061258.1+570222?ïþh÷Bõ§?ÍU½"?)pŽ"»yZ?ÍU½"?ïò€Fü²?^îoNj?Zÿr‹íš\?^îoNj?ïø¨V\b?@§cõÖ¦?M^§WÎèc?@§cõÖ¦?ïð´ßkŒ?Iýµ›?^–@{÷™h?Iýµ›?ïýrnSè?*Þ6ön?4lŒóåòH?*Þ6ön?ïŶÎ2Óg?ƒç¶ÛÍß?}$˜ï…H|?ƒç¶ÛÍß?ï÷¾" ?[üG%8âµ?P'×ñþ€?[üG%8âµ?ïÙm¼r??eC7ôù:¹?sIs"vÌ_?eC7ôù:¹AGN4FGL J0617.7-1715?ÐíÊ›¢¼À.!6ŎêêÀ9"#rËÏwÀ;Û¢4rÎT@‹-á
¡?üœ¡ž¥r?¶¢?/•ÄÎ?¼ÜÎ!¶‰@¹ÍÄC'O@v]ÃՂS?ïã3@Ÿ-¿àÅã~ê읿ÝÈ輗u}¿ÖÞ$Þ[À¿ÜàA>
ׯ¿ç=ý¼ƒÔAGNbll3FGL J0617.6-1717IVS B0615-172?ïùe*7rC?Dê<vÈÙ¿?JkV>ãþ?Dê<vÈÙ¿?ïìU–_}i?aÑš×?cªiØÜ.¥?aÑš×?ïëUÌÃÆ?iåóÅK,†?dª3KX,`?iåóÅK,†?ïÅËÙ)Hñ?W"¨ÚYqC?}}éke?W"¨ÚYqC?ïñ=)<v?ZvíE0íN?]˅³tÞ?ZvíE0íN?ï¶CxСC?†[b¹fF?'o!Ãð•_?†[b¹fF?ﵦ&S?†'Q%âg¿?'¹Öy–"Y?†'Q%âg¿?îûoG¿ý?'™20Ù'? IˆZ"0?'™20Ù'AGN4FGL J0618.1-2428?ê"#ÝøÀ1՟+©ÑöÀ:Žîr9€À<Q·åž@ñü"up@ÅsS6?ÊvófêoË?Ê\o—'ƒP?ûëlË@5'éþâ¿çzŠªéM6¿Á™Ãàêç¿åÈÜä.¿ã"I,«¿íÁÍÊùö¿ï‹›ÿûMiAGNfsrq3FGL J0618.2-2429PMN J0618-2426?ïÐY˜¼hÀ?r—TDKƔ?wÓ3–óê?r—TDKƔ?ï詏ZüP?iÄAoU]?gVp•åh#?iÄAoU]?ïy"ƒb ‰?'Õ
M&Ê}?Û¯<Rá?'Õ
M&Ê}?ï´Õ(¿Ã?cV‡zh•?'ʵáoçZ?cV‡zh•?îøøWü&"?™<—Rd? pz}©á×?™<—Rd?ïžãõ!C‹?'¸…¯y?ˆGÅm?'¸…¯y?ìîC÷?€ã?§
·dÁÜÀ?¸àFøç?§
·dÁÜÀ?î¹µüã?˜ì|xH'?®äoD 1Ó?˜ì|xH'AGN4FGL J0618.9-1138?ï»Ê0@ªÀ(Ӝ"öœªÀ:%'ºZ'À;±B¾ÁqO@¸w¿T>F@	1)Ì?Ïåwh—C(?ӊ©|:¹@W
"˜±<@
¯î~Î<¿ÞUµßJ}Ó¿Ù@½!Þø¿åÒ!ÀšŠ¿ëò9Wÿ›¿âÔrþ¥7¿ïÿ­AGNbcu3FGL J0618.9-1138TXS 0616-116?ïúJ=³6E?BFjsþ¦?F×	¿Vú†?BFjsþ¦?ïòIʊŽu?YzŸ±Ë9†?[ljfò¤?YzŸ±Ë9†?ïmMƒ@'Á?‡"õÏxÄO?'VO—íÇï?‡"õÏxÄO?ïð…Bck¤?C!{ÜMñX?^õ{'·'?C!{ÜMñX?ïøi
4ÆÜ?O÷o%Í
?N[˂ß?O÷o%Í
?ïȒцùb?"Ð#)¶îÐ?{¶—*¥WT?"Ð#)¶îÐ?î#=w¸Pò?Ÿœ…ìšpÐ?­Ì(€/mß?Ÿœ…ìšpÐ?ïdŒ–ž4?ƒgÐƙé^?"nm*²?ƒgÐƙé^AGN4FGL J0620.3+3804?ì¾Ïµ¤+@%|L7æ÷À:5ÉæhÀ;™4A@3X¡¬¸…@#ŒÚnuÿ?ÎP¹ŠÖ³?'£7'3 –?Ñî¼t@`­Eîé?ì8npöã!?Û{ļ²ù<¿éÓ¯ºmO¿æ(ýð[GN¿äêîU³¼¿ïÿöZdÐdAGNbcuGB6 J0620+3806?ïâx}åo?r`h¹"A?m‡ÿ´ôÈx?r`h¹"A?ïµÍ€Àž…?Ž¯0eÀ§?'ŒŸÇñDË?Ž¯0eÀ§?îf"Cqò?"o¡F¹?©—»Ê¦>ß?"o¡F¹?^K ù?s—kLÅL›?'(bÈí²?s—kLÅL›?îaW}O°?®º‹Hm\?©êˆ.ï	?®º‹Hm\?îZ̨ Ù»?¶H4ß÷*?ªS5t:–R?¶H4ß÷*?ìY:±Â¸?«%;¨™š?½6*sñê>?«%;¨™š?ë33º}Ð÷?²;¿RÌ?Ã31¼"?²;¿RÌAGN4FGL J0620.5-2512?î}2•Ôh"À1™ºç£À9¬6KìgÀ;å &5@añµaÌ@]d_%)…?·ÈG¾àù?Ï°%1½½@WƒPù@KF?jú?·J@€x¶J¿ã*óÿ@½_¿èYö|É¿èæ	ITݨ¿ïÿé{2¦¿ÓÀâÞ±ü'AGNbcuPKS 0618-252?ïÙËvǘÂ?nݸÈ(Y?sD·"?nݸÈ(Y?ïñhä/§?\EƒLèf?].77Z"v?\EƒLèf?ï."Äâax?¤òÝŒ¦?š-ghÛ:î?¤òÝŒ¦?ïïÜBê}?Fn6MXWÔ?`#½êôºƒ?Fn6MXWÔ?ï²yŽûÂ?€¡Á&!î?ƒa¾,g9e?€¡Á&!î?ïËgwæôõ?{øäï©$?zLD#â݁?{øäï©$?쿄í»ø?¦Üâj‹k?ºؒ'àD?¦Üâj‹k?ïn¿^áH?~pL'N¬–?'(,nO?~pL'N¬–AGN4FGL J0620.7+2643¿í¥ÄF˜–@¯^AÔ¶¦À:¡…}'ãÀ<E-5Ã0l@#XÅq8Ò?ø‰{>d¿?ÀÜ gS¡=?¯pÐDÅ?ñ&'+½óì@<HQRƒ¿ïø½Ÿ¤v¿î¿ >ybm?ïÿ!ž5_³?xõá)a^{¿à
Ç9G¿œô"'|êAGNbcu3FGL J0620.4+2644RX J0620.6+2644?ïþ•f{x?ªKå5§Ó?&©™"õðõ?ªKå5§Ó?ïêìÁ?jë—rü?e÷19â?jë—rü?ï÷…ºû¥?[°Û/15?QâôÔæ$?[°Û/15?ïôó9žf?Gºä®‹t¨?V,?Gºä®‹t¨?ïþwa¶Sd?!ÑVYàêd?(‰áª¸ã	?!ÑVYàêd?ïA惛ð%?¤Éõtœ?—Ã/‰_i?¤Éõtœ?ïù\êð,?`›`zÙ?K†‹ð½Ó½?`›`zÙ?ïèÇ/1¤p?cadÄ·=?g8Ðå¸çu?cadÄ·=AGN4FGL J0621.2-4648¿îis¿}fÀ8]æ?À:×Fšï/À<{«?´Jö@€Ñ¯	ÃM@Ò>ƒÉM¼?Êõ°kϲ?ÀôºQ Ä?ïü"à՘M@Éf'0CÀ?ïԉ>؂ã¿å©é]|2¿ç)y
­Øì¿ë);b¬'¿ïÿ¾ú¿±€
A/šAGNbcuIVS B0619-468?ï´_¨(Ÿÿ?²§ÏV-ÍÝ?'èêÙ@c?²§ÏV-ÍÝ?ïçÝ-u¸?zÙü¨`˜?hþ"ÞèàT?zÙü¨`˜?ï¬V¤kI?vtÞ-@þ?~©Ô¦ë#À?vtÞ-@þ?ïÛ­§åÚ?X‹Ñ}É#?r)+û5ä?X‹Ñ}É#?ïûšà8ø?=©ÐkÔ²?A"‡ÏÓ?=©ÐkÔ²?ï¨ù~º"Ú?dNâ®ê?…Á Tæå'?dNâ®ê?ï'Ùۗږ?ˆÝ†ô?‹‰‰ è'W?ˆÝ†ô?îÝZ)'}?z&ØI?¢/ú_%V0?z&ØIAGN4FGL J0621.2-2213¿éãÀ¢-MÀ0LY§;BÌÀ:¸
!Áñ§À<vžy_g@"SCôÌp@b5deÛ&?Í/ÉÜ­j‡?Ï'쮤@=–é»ðÜ@Æi'wâ?íÌÙ,V  ¿äˍ Îí¿ã§".οâ.0y²É¿í*áã¿ïº«ÍxÄ7AGNbcuPMN J0621-2213?ïõˆëÿöx?Iª¢Ï‹,?Tî'ÆYŸe?Iª¢Ï‹,?ïñ°üÀ8?[/MT*|f?]òž"ñ/?[/MT*|f?ï­¹\~0?{*û¡?"'»%p×ø?{*û¡?ïÚµÒ¥¯?QãI¤Û_k?r¥+Hx?QãI¤Û_k?ïö&#Œ{?P27""wI?S³¹Ãj)h?P27""wI?ïÏvO4#?|DT'RÏ?xDØOùnÂ?|DT'RÏ?ï7ŸL"Ì?"LN¨¨¬ç?™hì
|?"LN¨¨¬ç?ïXÚfU"?xíäEx?"ä³8ö~?xíäExAGN4FGL J0621.7-3411¿ï°,ù2[rÀ4"D€bïÀ;ö¤À<‹S+ ?;@ L'Þœ?þZ˜⚔?ЙÇ|Uæç?Äx†$?òbI$.?ÿ‰®ww/â¿àÈA§õÓ¿î1­ÂEŠN?¹ú[?/¯Š¿Ýkq}›·+¿ãQf™'
¿âõÚã1AGNbll1RXS J062150.0-341140?ïýÜ+[ð¹?%Êrö-?1£F–€¼?%Êrö-?ïó7Giöê?YT(ºøÿ?Y'q)R|¬?YT(ºøÿ?ïìn£Q?b õY«?c'ð«ÂÇ«?b õY«?ïëzW4b?HÈ®¯bå¬?d…¨–L¶$?HÈ®¯bå¬?ïýíÓz?0—aŠœZ?7"Ì­-?0—aŠœZ?ïÊ­yå
$?…EÝkÖM?z©BïìÊ?…EÝkÖM?ïæۖ¿¹?oÂûzM»­?i$i@áF¬?oÂûzM»­?ïŸ}16·U?wˆþýÝ¢?ˆ ³¨VÜ?wˆþýÝ¢AGN4FGL J0621.8+1746?á¢gÆ/F6?ûyŒ³Ø	AÀ:¬¬ÊÎÅËÀ<Û£)eT@!å°²9ùv?ýË?.9?Ìa2µ^ñþ?­Í bSºÆ?áxg_µ0@<¹y]å?¶ÁŒ@¯aq¿ïÿ…ãp?ïáeáhö¿áQÛm¿ÐÄށU*)¿Ù\+d‡¾üAGNbllRX J0621.7+1747?ïþ̕´ ?)'7".T?#6¨|¼Y|?)'7".T?ïéÖÎ-u?t¨»P¶K?f)2#¤o?t¨»P¶K?ïõ·d…»–?d4gÌ$(Ò?T'6ä
³?d4gÌ$(Ò?ïúP•¼×?6*%6ÄqR?F½©õœê?6*%6ÄqR?ïÿ,,ÑÌ?Z/p­‹"?zk]F"*?Z/p­‹"?ï#)ï×W¯?ª!gˆï5)?›šÂ]<"?ª!gˆï5)?ïöôݦӃ?cú©½/?RD>æ0?cú©½/?ïó†(˜>?S¹BÈp?Xóù݊2ì?S¹BÈpAGN4FGL J0622.3-2605?ÎÐ53_öÀ1ŽPÅë1<À8w¬-ðÔÀ;¢ªùš‹@ûNuÙËä?ý÷dñ`¯?¢¡È€üƒŽ?
YJI$a?úbxÐÌ5Î@8xé@¿á䥜[d¿ØqCå+B¿Þåe_€C1¿ÝÔY¨‡s¿ÚðÁ^.´s¿Þìþ¢˜œAGNbll3FGL J0622.4-2606PMN J0622-2605?ïÿC-Àò=?	 `ÕœZ?šD¤?ªº?	 `ÕœZ?ïö¸¦–?R¢æ|§Â'?RÂNdÄ?R¢æ|§Â'?ïïžré£ê?pw®Gï?`aMUÕ<?pw®Gï?ïÿOàÏ<?˜ÕåûIÓ?ëqÉ®D?˜ÕåûIÓ?ïþs_7õ?!ÙiunŽ‡?(Ê
'?!ÙiunŽ‡?ïٜ•';?µ>ì	1?s1µ%"}Œ?µ>ì	1?ïà#èMÂè?n¦c£?oÜŠa Š?n¦c£?ïÿ!GųË?¯l&Ö?×¥5?¯l&ÖAGN4FGL J0622.4-6433¿ãp»Ô×ÞÀ;bÎ-±êÀ:»ƒÑÀ<W0º²îÕ@zô»Ô,@¢¶®}Vm?ŝßN"¿°ÊkÞöE?å"Èy€õ^@'~øƒ‰ã¿å@¯½ÈM¿æäÚ_²m%¿îA¨v¬.È¿ÒÊrŸ¯³6¿ÐgÕÒ/¿ïýßßy!ÕAGNfsrqRX J062308.0-643619?ïüEý Ð?EzÊVgµ?=Ð@¦¾¼?EzÊVgµ?ïí2Yr?{Œ÷E®wX?bÍå²ì
ß?{Œ÷E®wX?ï²¢ü¼ $?ƒ¥¦Îy‹?ƒW@Ãés'?ƒ¥¦Îy‹?ïýχ£^%?#ЕòœÜ?1ƒÄ"²@?#ЕòœÜ?ïùbù¹-Í?Pà.îpܚ?JtÝåܳ?Pà.îpܚ?ï¼wA)@?‰x‡ðµ?€â8â§,
?‰x‡ðµ?ï3pQ?‡¦G &Æ?ˆ³:¸4OÃ?‡¦G &Æ?ïÑ?ãz'?tΏwÖ?w`qÿ$¤?tΏwÖAGN4FGL J0622.7-4141¿Ð…3ÇløÀ6¸¼M"ÉÀ;Ć­-ËÀ<ØmSÀqu@œêxÚ1d?ÿ¤2‹m‡?ÈeŸA#`Ø?ÛKkä)µ±@g ã¥Vf@ãNòï¿ïÿûÎBÓ?ïÿÌÐJ†¿ÝÌË_ºOÈ¿âqß«Ì¢¿ëäò}¶d+¿ïÿå]½JyAGNbcu3FGL J0623.1-4143SUMSS J062242-414357?è,:ª¤è?Âø'•˜«?ÏOUÁl`?Âø'•˜«?ï8ªÕ
?ŸK{©'?œ˜ê±´úe?ŸK{©'?éNS˜Œ?°žx~"o8?ÊƱÏç½?°žx~"o8?îŒ7¯!sÌ?‡01LÞgð?§<…
èÃE?‡01LÞgð?â§6'?Éü¤°ïÛ?Ú±õ"óðÜ?Éü¤°ïÛ?êTqFi?Åɉðõ?ǽ®:æ[?Åɉðõ?ÑóÚF¡¾Æ?»a«E€¢?çܯ ?»a«E€¢?æí9¢@º¹?µé]|1ÿ¬?Ò%Œ»~ŠŽ?µé]|1ÿ¬MIXED4FGL J0622.9+3326¿ä¦Á}¨@"MŸ±áŽüÀ8k"ÌÐÿÀ;fr° Ĝ@VfXN ¢@D:Âs­? §?ä5bý?´8p)³®@KïIÏVë@azXᘌ¿ÑI
`EË¿Úölmçd(¿äÿ­õœ¿áWÂ~ë'¿éB=äg¿ã¶ô›»³AGNBCU3FGL J0622.9+3326B2 0619+33?ïùI(Ä?En!sÕ©,?KÎÛÂ&<?En!sÕ©,?ïèÎØë"
?q¹©€?g1'6È
"?q¹©€?ï½sn-õ?'½}	Ò"?€£?ŸýÔ?'½}	Ò"?ïÿâEÚÕ¤>å–,ò}'>í¹òAb>å–,ò}'?ïõ$©Fy¦?Pv¯¬g?U¶­¬Æ$?Pv¯¬g?ïhH[þ?¥°ÑìÓù?'þ6÷ïØn?¥°ÑìÓù?ï
>qL?ì?—.CÒk0ö?žX1Ϙʋ?—.CÒk0ö?ïÿÖå¼]>÷¢Þx×ɜ>ôú$AÜÛ>÷¢Þx×ɜAGN4FGL J0623.0-3010?ã÷ԑ"ÛÀ2ëèPïÝÀ:Žf5¾þ®À<WoŠÑ€@sªZ1#ä@üCbU_®?Çy-¾T9?È´͆†?ÿ4i^hk#@	—49˜}¿ï©\ºëù¹?ïþ•œ´×
¿çýŠ¥
$¿æÜþ]¾w¿ë>ÝöÀ¼¿ïÿå(
eCAGNbcuPMN J0623-3010?ïôrïœìœ?TݬýOO·?W kqs?TݬýOO·?ïõ"bÅ5î?VPò–ýá?U»:œÂú?VPò–ýá?åxa³?'­GgšÞ[?ˆÔ†³Ÿ,?'­GgšÞ[?ïõ‰¦KG–?<?ÈÈ©M&?Tì³[²d^?<?ÈÈ©M&?ïõ4©;3?XäVú3G‹?U÷–Eyµ?XäVú3G‹?ï×ÛRîܹ?t®c+¦¨r?tVk´ëm?t®c+¦¨r?ï	èëŽH?"ÑÌb…
Š?žÂýbŽ7?"ÑÌb…
Š?ïÈ#¤í,5?pHÑ­ÿk?{î-¡w)D?pHÑ­ÿkAGN4FGL J0623.2+3044?ï`ÕðYfE@ ¨½#žÀ9Ù©-‹TÀ<E¢Ë@ ¾!Š?üS€*\ÊÜ?Àµs>æð?Ä=ʗ"Z@'üÕ©@&ïjÜlÓ¿âDrØ
¿æBw©"É(¿àø]©ÿBk¿Îêq"'¿Ý`QyoW§¿ç®Žd•AGNbll3FGL J0623.3+3043GB6 J0623+3045?ïúê%‰M?WÁ_KŒÙ?DWl¤ÝÅ×?WÁ_KŒÙ?ïã²h!?v­+›´ñ?lûM®~—?v­+›´ñ?ïí·Â4Ԅ?`1îs¨Š?bH=óó'?`1îs¨Š?ïæf±Ú~?M–평?i™N=KJ6?M–평?ïôǜP?S,6úÈõ†?VpÇîŒ?S,6úÈõ†?ïDÊ\&"à? uh0ùƒ?—f´'»ù? uh0ùƒ?ï"+•HëÆ?Œ$ð÷º¼H?‹5¦å֋?Œ$ð÷º¼H?ï†>Þb!?y¸™,ÂñÏ?Ž~pD÷Ûã?y¸™,ÂñÏAGN4FGL J0623.7-3348¿íÈô&Ç®ÅÀ4[À6ãÀ9ìuk¼ç|À< 9€
@ Z¬Hóº@bê¾O[ˆ?¶Ô? Á†?ÆÌV»£…@ºk
F@ëc`w?ïeáÜ(Š¿Öæ€',À¿ääµ Þ¿ã²æ!1¨ï¿ë"Ÿ»Ì¿ïù)ÍAGNbcuPMN J0623-3350?ïëŽøð…þ?ayá
?dq5õ¡€?ayá
?ïõ'üä?U\ý1ê—?TÜý(Šè?U\ý1ê—?ïR0«]U4?(ù'ê(ô?•¹ê'‹s?(ù'ê(ô?ïûÈ}²³F?&ËïÛ	 N?@Þx5‡?&ËïÛ	 N?ï½ÌQ&ä?'ÜL™!(ä?€Œë¯Ën?'ÜL™!(ä?ï؏܊¼?wšL?U?s¸¦[ùð?wšL?U?êì~1DË?®œ
²ˆß?ÄN:íøÓ?®œ
²ˆß?ïñò†¤õ?H`Lz?\ÔC6?H`LzAGN4FGL J0623.9-5259¿æ¬ïH'ƒÀ9[ѼrâÀ:è	¬Q,BÀ<£O•i‰1@yfÞ±PÅ@Á¶ža?Àd鎤s¿ ©Ü1ï'H?ãæ¹Ù«@K^ù	¿ê''Ò¬á?…pU0ð¿ä&½2%¿äO%‡N"¿Ò3f~¿á> AiõAGNbllMS 06225-5256?ïþÂ_
§?§­"Ö($?.£Ý‡½Pn?§­"Ö($?ïöy,wéW?Ta‹<2?S
¦½¶²Ä?Ta‹<2?ïä÷R©½v?sæka?k­yþz@?sæka?ïüMb"MÍ?#ïH¡ï—?="ðYÓ?#ïH¡ï—?ïú'T>??1ÙU
[?E·ã3GIž??1ÙU
[?ïב#â?ƒ1ހ¶%?t7nc°]'?ƒ1ހ¶%?ïìN+Í
?mÿ…"'?c±r©—Ê×?mÿ…"'?ïè€×xCÖ?[>|þ[w¹?g(¤˜áó?[>|þ[w¹AGN4FGL J0624.2-2943?ÓÁyñnÔÀ2ƒ`¦3À;-Á>#Q>À<šnkîe¤@ g
Tý2p@2fâ(r?Æÿù_|è3?'îƒx<t?¸paö"@íW<ý·P¿Ô5k×ÌÛ¿ïÕrùà0?ëFúû´@å¿ãÚ­Ëų¿ê&ÏAò×?ÌJry\ãAGNbcu1RXS J062422.3-294449?ïù˜ëô°?[ã–w¯Ç?Kí›iG€>?[ã–w¯Ç?ïõ³Ù5æÂ?X'h±?T˜Mº®J?X'h±?ïÓfU/Ãx?s'L'x0?vLÕTàsõ?s'L'x0?ïñžêL ©?M¡ÅXÆÐV?\Â+[¿î"?M¡ÅXÆÐV?ïðÖ\˜‡?]¿œÃ2?_âS('a"?]¿œÃ2?ïÛÚ㪣œ?tü°ê¹?rŽ4Mý?tü°ê¹?ï¼øPߥ?ƒ7iœ#~4?€ÁëÐ!°Ê?ƒ7iœ#~4?ïØæ,¼™?k«Í 6ã?sòŽ/]?k«Í 6ãAGN4FGL J0625.3+4439?ﹺDm¡@,Èdìé¢ÆÀ9p-ô/fÀ<-ëÎð"{@+'þKË@j0¥º9L?®Š°av|?©|ýÇ%C?úÔ:I§é¾@
8
û1¿Þi"$a¿ÛQìüíüÈ¿áÖ¸ÞÙ>Ë¿á&ƒÝo²@¿â¿Ð/WÜ`¿ãºû~ÿ—AGNbll3FGL J0625.2+4440GB6 J0625+4440?ïþ>(§
"?k%U@–?,y1†§·?k%U@–?ïñ:±Æzè?aÎíõw¢	?]Šœ™…Ïò?aÎíõw¢	?ï÷ñô®??Õy¸õk?Pû"ä??Õy¸õk?ïò&x(Ÿ?EÞ÷C͑?[ã³m1?EÞ÷C͑?ïüýŒ]F?-Kây}?8›J7k¨?-Kây}?ï±%æ³A¥?‹Ô¢a‰ö?ƒ¶†Y¶Ø¬?‹Ô¢a‰ö?ïö¸zt)6?`Û=¦pA?R
™;óÈ?`Û=¦pA?ïÕ¬eµLº?cœEØ÷Z?u)Í‹oB?cœEØ÷ZAGN4FGL J0625.8-5441?ì¶8:ÈÀ9o¿aª?À:5C•%À<VH˜F@Úäå@o–@HÅl?¿o"͊aî?¶šÇ—æd?óƒ
€òç@	¡hðÚH?Ë&`¼Ù9ÿæk%^¿ê«ᚺ+¿ãu"Ód—¿ïþŒÍÙ<G¿ïô€d{AGNfsrq3FGL J0626.0-5436PMN J0625-5438?ïý›˜ï?+‰¸ç
9?7$ºpϔ?+‰¸ç
9?ïõØØ*h?W&¸?TOðbéM?W&¸?ïé,ÇyÒ?`—ž°oF?fÓ÷Ubæ0?`—ž°oF?ïóä	ÄÙ?B³­Æ2[@?X7ìÂÞ&?B³­Æ2[@?ïýÒÕ\?282VN]?7qjv^R?282VN]?ïÕÑcñ}?"ÃѤÆ?ut—jãù7?"ÃѤÆ?ïßÕk_}?zuܽŸ?pJpÅõ?zuܽŸ?ï½+ŽÆyC?o'ó31V?€µM×A?o'ó31VAGN4FGL J0626.4-4259?@1skÀ6qgÛ±lÀ:gØp¤®À<rZؓªl@ =é[;e?ùXñ°C?ÑIÓގì?ÊGçµ±RH@'í]f¤@-æ–Íar?èM!*È+¿ä'%ߍš¿áŠJ;tÈ¿Òu.`µ*¿Ü4%áæåR¿éäóiï‡ãAGNbll3FGL J0626.6-42592MASS J06263670-4258059?ïþ*ªæ&?!
"Œ'ˆ?-Vô"&‹í?!
"Œ'ˆ?ïöBÜtœ?T@ŠMèƒ?SzGy#Gý?T@ŠMèƒ?ïëðŒx&‹?]µýú€‡ú?ds –¤ü?]µýú€‡ú?ïü2ї?!øº½?>irœîûX?!øº½?ïþu4p±)?$'tM=]?(¬¼-m?$'tM=]?ïÓ£¾ê¸?í
x{I?v. w¸T
?í
x{I?ïÜ £o?xc҆ÎÒh?q¯õÛTˆ?xc҆ÎÒh?ï÷Yƒ)Ì?@uö}Ђ?QLù/dÈ0?@uö}ЂAGN4FGL J0626.4-1712?춁	»ü¬À*FhEZ}À:¹%8ž¬ÿÀ</½ÿªo«@<ä1˜Ss@<à[?Â¥ýÖ.
¿¡K×ÄÍyñ?àwU6":@bÀõ(5©¿Â$ޜ-Ä¿æb­¿keT¿ê'v¹Ã?²Ò<ççÛ¿ç+Zâ#Ì
¿áã+~3ÆAGNbll2MASS J06262650-1710467?ïûè:*b?7Ç`ªüI½?@_üN­?7Ç`ªüI½?ïó¥þúø?Xãîe˜¸?X´Ì¡?i?Xãîe˜¸?ïåð™ÒñÌ?n+ãòÑîÉ?jf9l˗?n+ãòÑîÉ?ï÷¯—í/?3ÌF#Tµ»?P Ò ¡"?3ÌF#Tµ»?ïåªL4ê?l:~óz\z?jUæ˜N5°?l:~óz\z?ïÎEE·ø³?€Ñز®s?xÝ]´Ò?€Ñز®s?ïºÆ²×XA?…îa‹Ïñ3?NSRÀõ²?…îa‹Ïñ3?ï¦,=åX?oŪk'Z?~¬éÿIä?oŪk'ZAGN4FGL J0627.0-3529¿–ËÆts8À3ø2¹¯æÀ8êe˜ºÀ;ÚꃖøÕ@è7cnU?þM€†£Ð?¥I['Ý?'AÒiCæ?ìf¡t¯T@– 5T –¿¦áÃ\"31¿ßZžœ¿Ç¿à[Õì¿×Â"µí¿àŠEžoÂ0¿àæÂÂ1é1AGNrdg3FGL J0627.0-3529PKS 0625-35?ïþ'~Ô,¤? #9@÷Gy?&èy
Qø? #9@÷Gy?ïõ´¸,?Y5¾âWÃ?T–s,÷Ë?Y5¾âWÃ?ïç³û<W?z¬v—iD8?hL†±Ð?z¬v—iD8?ïõPð;?DHRÍ×âž?U^E²?DHRÍ×âž?ïûËy äb?:p
²,Ò?@Òl¬¿?:p
²,Ò?ï։vXCZ?€OîÐ6Ê|?t»DͯÔ?€OîÐ6Ê|?ïïý-_++?q¢ü€Vð?`ÒÈ°Lª?q¢ü€Vð?ïꘓppè?ZŠ\Ëïƒ?eglÃÉ(3?ZŠ\ËïƒAGN4FGL J0628.6+6900?ÔK/.Òâw@75`A‰7LÀ:¶çºŽÜ§À<¯Tæb4@°´k½@j= ÿ:?ÀF¨0
_?¥0¼ê½µ?åAa)ÃÂ?üPåüéö¿Ç?›5ûåi¿ßN€2ÀG¿Ýߋ€Ò"w¿æîâ q¿àáÕ<ÝÖà¿å¢zH›zDAGNbcu3FGL J0630.3+6906GB6 J0629+6900?ïù£ð_£ÿ?Hˆ¿i-9(?Ip=ÝÍ?Hˆ¿i-9(?ïîxõÎè?`ÑìZªp)?a€†òÓ¿¬?`ÑìZªp)?ïä0å×(?kC"ŽøV?kÏÆj?kC"ŽøV?ïÉË¿AÚý?]f	:6•½?{ y/‰`?]f	:6•½?ïêѪø<?Yg2Ï@0¦?e.î5k\p?Yg2Ï@0¦?ﮊŒ,ëé?…ÞRæiÇh?"]]"9»?…ÞRæiÇh?ïÏ^b¾Ö?~A"Yiqi?xPûç]Äò?~A"Yiqi?îßÎÁl?ˆïUCñtá?¢¯¼ê?ˆïUCñtáAGN4FGL J0628.8-6250¿äfPxWCxÀ:vø½ì_9À9—Ú\ØHÀ<]õ£…«¦@Ûwy´!@ä̂úñ£?²ñLˆï¨D?¸¨xY­ñ?@GË $b¶@i}G(‰¿Ü¹­6/¿ã/¸ToÃÝ¿àÜßõÉp¿ãòžþˆ[¯¿â.•ßе¿ïÿîͨ"ßAGNbll3FGL J0629.0-6248PKS 0628-627?ïþ5Å+:8? G׏?,£¬Êžv}? G׏?ïõ‹
=NH?Y2얊©?TéëèX/ø?Y2얊©?ïë TÓ[?m_hY©iC?d_ÿ¢í•A?m_hY©iC?ï÷ÒەΚ?9þøL˜îÛ?PZHâgš.?9þøL˜îÛ?ïý)ÐC¯?0eR‡ R?6±€éJž©?0eR‡ R?ïÚ¡V|c~?uÖ(}¼7?r¯T° 5.?uÖ(}¼7?ïà³h;—u?xÞ7kñ§?oL—ÀIq?xÞ7kñ§?ïãŒ÷õšv?]€ÀuI¯×?lsûGA²?]€ÀuI¯×AGN4FGL J0629.3-1959¿è "ôûÀ+U›=ÈKÀ8¦$'–GÖÀ;ŸñvÐ@ö@í®Š)@/L{ٕ2?¤þ€_G‰?²{婒‹@7b|×Â@¡ù5‹}!?îÿ5Ÿôým¿à;Ø»¿ã죗I]A¿âYÿ ^¯¹¿å•[|'˜Ë¿èK×nç>hAGNbll3FGL J0629.4-1959PKS 0627-199?ïþŒÓ­?G81\?(5æÛ-›?G81\?ïô@€ðøž?]pfäøR?W~þƒÃ4n?]pfäøR?ïï"wh8Æ?XíDŸs?`kˆÆéÙ?XíDŸs?ïÿUÌ¡j?'ñË_N?Fj$ž…Ö?'ñË_N?ïþ¤ïŸEç?ՍÃXÖÍ?%±‰Y
(?ՍÃXÖÍ?ïиÚ|Å?…Šç´Œ?w£'©«Ù?…Šç´Œ?ïáƒ$"'?v0ýx&…?n|ÛEÕ?v0ýx&…?ïþì†?c‡?Rõ	Ëq?!7šûL¸?Rõ	ËqAGN4FGL J0629.6+2435?ïâŒxã…e@ë—¦zSÀ:w,50"À<6¯A@ ,IõÂdi?þ§,yێ1?ÆÎ'€L–‡?ÊÜ >ú;Æ@Ó#þâÊ@`KZS3¿ìõcߣi&?ïû0Ãj¦?°\ڗe¸¿Ü¨
»)Œ@¿å­Œ?¾ÜÊ¿åÁЄè1­AGNbcuGB6 J0629+2437?ïûUúf¼?7þ‰2'k|?B¨ÿ|x?7þ‰2'k|?ï×B§D}?wì^ßE·¦?t^¬I#ÔS?wì^ßE·¦?ïçS_3ÓR?_ѱÈkgx?h¬ –'Åì?_ѱÈkgx?ï»Se'»²?`ñ09oÁ'?+&§8-Ž?`ñ09oÁ'?ïöG(ß?P.s~ʧü?Sq¯Æå'?P.s~ʧü?îÓw½À".?­ü—OC?¢È""?ï$?­ü—OC?ï€ó/l?kŒw'¹?Ã4#œ]?kŒw'¹?îì!!žòZ?Šrb÷ZºÃ?¡=íã}%`?Šrb÷ZºÃAGN4FGL J0630.2+3228?èTÊZÒc@$4D‡BÀ;Mä·¥[À<}Pǘ°@ ÿ€Êì?ÿ°g܈+³?ÏMyÛc='?¶"¾ì†?é\>ŸÍæ@Xg‰Q"¿âÄõ"+y?î°LÎå«Á?æÿN)X¾Þ¿èY¹Å¿à9™m$?—àèžË˜ÖAGNbcuNVSS J063010+322608?ïþ!—eû?"õdi`¿§?-æ‹ï?"õdi`¿§?ïå¯Ñá«ù?vƒ^ü¤C?jP.vÅ?vƒ^ü¤C?ïæ
ªM?fŒ›Œ"t«?iòñü"ƒ:?fŒ›Œ"t«?ïݣѣB²?[o–k¾?q..^¦î?[o–k¾?ïýv1ycˆ?1dkç‰N²?4Nv6\v?1dkç‰N²?ïh"÷&?žQ#îx—?'흔àS;?žQ#îx—?ïÚ^:à¦?y±qwʐ?rÐâЬÅ?y±qwʐ?ï†t{|øú?µŽ°È
v?ŽbáR%†?µŽ°È
vAGN4FGL J0630.9-2406?ïS5b&‹À-ý˜ZÕ8¬À7Å™m#ðÀ;'>[…b@â³¹€iÈ?úw¥ôïp?›h´§ð}	?·³ìŸ@©"þ×áÔ@²¤­sì? Õú¿É¾¹ä'¼0¿Øtߚ¯Ä¿×{Ì¿‹Æ¿Û½ûx±Â…¿â™
'¡/AGNbll3FGL J0630.9-2406TXS 0628-240?ïú•ÀF+³?KÒ ÖX/?E¨ÿ™p$´?KÒ ÖX/?ïɱ	!ç±?‰STÓÑTÅ?{'{|ʗC?‰STÓÑTÅ?ïaõ'<t"?"…ûöé¨f?"ÁO±'5?"…ûöé¨f?ïÉoeœ¯?iŒ7Ã%-0?{HM:â$[?iŒ7Ã%-0?ïõ?y+~Î?\å²%}Ÿ?UuD?\å²%}Ÿ?ï":ó/?°ðß.Ø?›¸¡ ö?°ðß.Ø?ï°Õtò?‹~›fxZ?ƒÊºõa'?‹~›fxZ?îÿ¬ÕOl?ûEª)? 2¬ÁÒ?ûEª)AGN4FGL J0631.1+2020¿ãäр26Ö@gŒSâÖÀ9kÛq«>À;—Ìe÷@@غÿñ@á">¿?Áݚzj)j?Êâë݉2™@'%ùŽÌ·@ð{Dü¿é7FBÐ_¿Íñ<†C&¿á§˜úà¿åàZéZ¢
¿çÀØ!ê‹z¿ïü-ãhÅAGNbcu3FGL J0631.2+2019TXS 0628+203?ïíL.»?\øM	Å9ÿ?b³êƒìX?\øM	Å9ÿ?ïæD··^H?s/•àú›°?i»Hb¾¿Ú?s/•àú›°?ï¨ÛoÁ³?~"'Ew6x?…É$¹[-?~"'Ew6x?ïô	n,1?@â*O™â?Wí#ՀN<?@â*O™â?ïÚmpŠ›i?resMZËÛ?rÉG¬Cï´?resMZËÛ?ï×<ùkÍ?¨Ë<´#N2?ž…]bêX?¨Ë<´#N2?íj–YѶ?£ÒD%¶ØK?´«M2¼)Œ?£ÒD%¶ØK?ïÏ~GN?fnñÖk¹ç?x@ýk' ·?fnñÖk¹çAGN4FGL J0632.0-1032?î³ݦ0MÀ"ÞÁÁÖÐÀ9¢sۍZÀ;¶^	}@‹0k,ɸ@æ*C hÁ?¿Ø×á—?¼ô
ÔDe`?ú̺=~Ð?ùqï-Iå¿áí¾´Ü?¿áđ?h¿âJ/-êôÖ¿çaZž:Ø¿ì‰OŸz"¿ÚCTþßïiAGNbcuTXS 0629-105?ïæ#ð	?fÇ¦×?iúÛÏYO?fÇ¦×?ïŒÖöy÷ñ?B9À¨í™?ŒÊBZ¢Ë¸?B9À¨í™?îF¸¾¢èx?{3Å,Ùù?«"t=Ç?{3Å,Ùù?Å:(½?ŠR3ñ¢ƒÉ?¦´3©É¿1?ŠR3ñ¢ƒÉ?íÙHî v?§RCiÎÅ?±5¿ÈŠüP?§RCiÎÅ?ì3B¸t¨?ÃÈÊ&ÝÂò?¾eê?¤Z¾?ÃÈÊ&ÝÂò?ìR(§ût?¨üm¨"Ì??½nºÀ'D_?¨üm¨"Ì??åi'ãÓ,@?¸kò
ï©8?Õ,ú8Y§€?¸kò
ï©8AGN4FGL J0633.4-2222?×OÂ]昮À+‰
Z[–)À:.MeÀ;ó£BÇ‰@Sϊí.@##—´½?ÁhÞ»·§?Ҋ¸?Ìô@"]Ä×5@f§€âéo¿åÛ1´­ò¿Ù§MKã-a¿æE'`À48¿êðÚ'ÿ"Š¿êŽ€á¼Èô¿ïÿ[ËñrAGNfsrqPMN J0633-2223?ïé²þrÚ?`gû¹·®?fMÞÏö!?`gû¹·®?ïóÀ'^$	?X*š©w?X±®ë½·?X*š©w?îÕ`ë/ìà?•Bù…Ú£d?¢©ñKIcþ?•Bù…Ú£d?ïûúêÂV&?'\šë¦ÚÄ?@Sì'tõ?'\šë¦ÚÄ?ïنR%Lý?pBî®-?s<ÖÓìeÁ?pBî®-?ïÌJN‹[ò?€Òñ;~?yÚØ¡"×<?€Òñ;~?ìâ›y©ËQ?¥máX?Ê*?¸ë$3Œu?¥máX?Ê*?ïåá£@ò?Z…PúRóÁ?j\Ä–6?Z…PúRóÁAGN4FGL J0634.9-2335?ï݀çFÊÀ+ë[³"ý*À9ŸŸ¡—[À;öюÓlú@b
#Ôñ^@Ì{n5h?¹²áØçQ?´Eæêk?ø"Ñ ¤<@ö"‹ë[-?´ãAƒXµ¿çň4íH¿ç>—"ƒ¿çÖ!ªt³¿ïÿŝƒ‰¿Î‡¾ bAGNfsrq3FGL J0634.7-2334PMN J0634-2335?ïûFoÐ?C]Y~è'?BæDaõkl?C]Y~è'?ïóƒғ
?Ylö|Œ?Xùü,;"?Ylö|Œ?ïäbÀâ?g:lFRg?kçðÂ>R?g:lFRg?ïæ;¯ó<?T|8"¤÷î?iÄPÃîé?T|8"¤÷î?ïøÌÔsN?IÏ-´k<¿?LÌ­ªp±ž?IÏ-´k<¿?ïÏÔ¢•Qò?~/#0•?x®•ºžð?~/#0•?ï̬9•‰%?€5'ø_?y©ã3+©?€5'ø_?ï]cöR?"ÌeÂ$D?"\ÏÖðѵ?"ÌeÂ$DAGN4FGL J0635.6-7518¿ëÅM†½ì,À;+Ë£!hÀ9"tnfæÀ<!™í|o½@ûPO£¬B@…×ÙôÓ?§zGÞÁp?ïé:g}?Ýò@úœñ@kº%€B0¿Ýﯛ
·ú¿ä†l@E‡¿égÿBÀÅ¿é»Âîýy=¿è;å¿ê¿á["{L§xAGNfsrq3FGL J0635.7-7517PKS 0637-75?ïÿ`x:Ï4?{•*ÂWÏ?ðø«Ý?{•*ÂWÏ?ï÷WjJ ¶?W¢M2½áZ?QQ+µö$•?W¢M2½áZ?ïëÏJ÷º?cºšù'Œ?d0ý£*NJ?cºšù'Œ?ïÿöWµžˆ>Ï»îå5™>ÓPº'2Ë5>Ï»îå5™?ïÿ¤H|Ï?qîK"z?íït¥'Û?qîK"z?ïÞ¢ºL?rÕ¯3.·–?p®¢ïF‡î?rÕ¯3.·–?ïØ|#Î!?yû#|Òӓ?sÁíüyÆ?yû#|Òӓ?ïÿñւ¿I>â©»_`2>ÜSH¢hµ>â©»_`2AGN4FGL J0636.5+7138?Çó`ר•W@8~´Øº@ÙÀ::ªù›À<[@ےbn@Eˆy`¿@¨[ü€¿?¹há?öe"?´Õ³{B¤?÷1^µ—ý@àl
ë?ïë!äVV¿ç5A•Ì…¿æwô˜Ã°Ä¿æ.ÕÀç;c¿èï9©nù³¿ï߄¬°AGNbcu2FGL J0633.8+7132GB6 J0636+7138?ïýèɶ•?!ý«¸eB?0¹´ƒã?!ý«¸eB?ïõ¼|ƒ?Y]£"Ê$?T‡FoUñ?Y]£"Ê$?ïíì:.Ï?M+!†?bÅõº!:?M+!†?ïþ˜<Þhè?(ŠlŽÌ?&|2x^?(ŠlŽÌ?ïüØ2±ƒ?-džvF‡­?9>lÃd"?-džvF‡­?ïÑ_²??{¸•Y'K?wqÐe<š?{¸•Y'K?ïá¦y.«?r%ÔIq¤º?nY†Å½=?r%ÔIq¤º?ïý4t•˜?'¬élü j?7v[óøš¡?'¬élü jAGN4FGL J0637.4-3537?èámz½	À2	t²GÀ:ž—•}À<xŠ]¼t@tècV;¡@
Ù©T"?ÆÀéª(2#?ÃuG?Y²#?øB*aÓY¯@2Ot\sH?ïÿôÂ_5›¿Û‹4œ>ån¿ß<߆d¿ç&zü	¿ßԜåS\¿ïÿŽ‹HÿAGNbcuWISE J063746.40-353648.3?ï÷&ó3é¼?N:§¿¸8?Q²šì7?N:§¿¸8?ïì:j¬i?esê™éØ?cãŜ2ÏV?esê™éØ?ïÍÞÆ°;?pÝ ?â)g?yœ¿Å¦‰?pÝ ?â)g?ïÐä–íí¯?W½Í>õ?w´ilÀÊ?W½Í>õ?ïÓÝ3'Ö?sػɔf?vfHI?sػɔf?︱åjÓ^?‡'<ȃ?Ó†¨
ؚ?‡'<ȃ?ï'¶$¿§ö?"EÔrÂ?›	;iÂÏ9?"EÔrÂ?ïe&[š—?ƒ½ÿú~D?ó[6D{(?ƒ½ÿú~DAGN4FGL J0638.2+6020¿Ûl›ÍYQ@5Æ՝Uæ¼À:Þ%‰ýDdÀ<'û_‡O@&cõÑb@ÿJ˜ª†Q?Ê"кm#Å?Íf¬¸ZO@ŒþùoÃ@hgÝ	¿ìÿº_⾧?ïû';&F¼¿å½xÁ‡Ê9¿æü»bJš¿ïöÃÁ5iï?Ä1ˆ8HEêAGNbcuGB6 J0638+6016?ïïtH7?aÂw\£‡?`ñ‹áÂV?aÂw\£‡?ïÙê‡rЂ?våjž˜ê?s
¼9‰;?våjž˜ê?ï¢!Ìó'?}ÜW8%?‡wŒÆ¥Õã?}ÜW8%?S؉?i©ÓÿÛ?‡R+œ.?i©ÓÿÛ?ïÛ[`×cÝ?r&ú	ÚÁ?rROua•—?r&ú	ÚÁ?îǶw)?³©Lü†C"?£Žh)s?³©Lü†C"?î.>#H§? yËW·?¯=§•? yËW·?ìÞ_‹½Û?¥Â÷ÍAÂ?¹
¦V*)?¥Â÷ÍAÂAGN4FGL J0638.6+7320¿ïûÍÈs@9ºùe²À:ó˜éprÀ<Mš#×v@!T‡ÁªÛ@-»Å=ŒS?¹¶2‡?xmّ2ö?»£Õݗ E@•§ˆo¥ª¿ã€¹ÎÃG¿ç¡L'HD¿ë¾Àdß}©¿é£"î^íÌ¿î6±•+v¿ï«WÂ3Á£AGNfsrq3FGL J0638.6+7324S5 0633+73?ïýùÖxЪ?*d[%¹ô?01KC0L"?*d[%¹ô?ïöçÛúoÑ?TØacóÉ?R0HpÔÍÑ?TØacóÉ?ïÜSÄçêÏ?n¤~îÖ3"?qÖ…+`q?n¤~îÖ3"?ïýq¥Lx?$™8êÖ\6?4rÙf@(?$™8êÖ\6?ïúѓ
Áè?Hàøz¬[9?D¹´'<è?Hàøz¬[9?ïÕµ×ÆX?zÎÿ¦l§?u%½¤?zÎÿ¦l§?ïÔef¥ë%?|ÓìNcå?uÍL¦+5S?|ÓìNcå?ïô
¥Hé?Làkgb³?W䵏*@?Làkgb³AGN4FGL J0638.7+2753¿Ú%§TYc@##_€™À;K§*{ԍÀ<œLŠN@!Y¹óA‰?ûø=^/`@?Ñ&ö¶|?–;֚ÖÛ?õ~…&E'?ôkڔ5¬Š¿ïÿï¤h)µ?è%¿âÙ~Œ?ï÷€Õ}uw¿åR÷Ù.Û¿ã×ýsº?Ë‹i*;AGNbcuRX J0638.6+2751?ïþþLå?(\öê6¸?.ð›YªÇ?(\öê6¸?ï—uï_7¸?"¥WN+Ã9?Š""$Âv?"¥WN+Ã9?ïÈҞ6Ñ?|\6N_;?{–°Êzo'?|\6N_;?îôB¦)C?ŠºI܊3? »Õœ"ÄÏ?ŠºI܊3?ïúûNÈîy?B$s(%Ì?Dij
ÊW?B$s(%Ì?햙Î.?ºl6R*!ð?³K1µ‰(?ºl6R*!ð?ï©ÂWd&+?…¨­žä?…j-Õ­?…¨­žä?ìÙ>Js?¬o• KöŠ?¿é6¬g?¬o• KöŠAGN4FGL J0638.7+5658?½Êž@4ÓDZ¢äÀ;
X;*xzÀ<›b§K3@¡)œ±|@¿¤Ùš;?ΐ¸‰ôµõ?ӜqeHO@‹"˜€"æ@¬@?¶#h?ïî¤!²Ø¿æUïÝëÙ¿é(ÒxÞ¿äœ¦°)¿ïþ–¾ßú¿ìÝE ž³AGNbcu3FGL J0638.4+5704GB6 J0638+5701?ïõDr ±f?OÚŒÿ|?UwԚ´?OÚŒÿ|?ïç^'õˆ?f˜¤m¾?h¡nÌOÈ?f˜¤m¾?ï¨ù|"a]?w«ß9‡pW?…Á Ð˜Ôæ?w«ß9‡pW?ï¿«¡®æÞ?]:mì¯b?€ŸE?]:mì¯b?ï÷'h$¬ˆ?RO˜TÜ6ˆ?Pû/Ý"e?RO˜TÜ6ˆ?ï?H6È?~ÅК'?Œ8ð 3Þ?~ÅК'?ï\ýãßÒ¨?¯nf;Ó~?"`C‰-?¯nf;Ó~?î<Ýï	Ä?'¹N˜±?¬2!ÿ—Ä?'¹N˜±AGN4FGL J0639.6+3503¿ä^à[R"«@)í¢Pø@À:Yã|;ºÁÀ<(ѧýàk@2Pó€Ý@9{ßto>?¿0öíݓ™¿ª¢ÒÛãÐ?ëu'Ìö¾@\T‹GœL¿á˜
þEjÿå¹ÝaD"ƒ¿ì/s‹¿ÓÄ{ÚìË¿ìÈ÷?½X¿Ä	´Ÿ.ƒ÷AGNbcuB2 0635+35?ïñÍ!RØa?TÉc9¡éu?\e¼ÿ™Ž?TÉc9¡éu?ïïúØÍ?_W9¬ù=?`ûF!Â[?_W9¬ù=?ï»WPì#!?'z.·#ö[?*+ÉnµÌ?'z.·#ö[?ïö¹[ð…}?<ß®å¹oï?RH¨4€?<ß®å¹oï?ïÙ5'¡|	?nL9µrƒü?selµWæ?nL9µrƒü?ï‰O»îÇã?'˜4ŠcUA?¬w&?'˜4ŠcUA?ï™"?Š·×ĸÜI?‰½÷sžÆ?Š·×ĸÜI?ï"Ø1å?èNuëR?‹	øpLjÓ?èNuëRAGN4FGL J0640.0-1253¿ï•À›ˆ~ŒÀ ¤€¥¬ÍSÀ9é/bÄwÀ;õ­§m—³@""†ÖHv'?ùÜسŠÜg?»~b MÓ?¢6,"9Ø`?åÛb'Ő?ù×E÷†	¿éx¶Ë¿åªy»­Á¿àY!95«³¿Î¹©™ìУ¿ØÃd£î‡2¿¶@¼ž+y«AGNbll3FGL J0640.0-1252TXS 0637-128?ïüÉ\Tê"?-´õ'šä?9µî4—?-´õ'šä?ïëye!'?fá¢'úÉ?d†šù=«?fá¢'úÉ?ïތý¡Me?siìwô2?p¹(zÇ?siìwô2?ïÕugáÐ?b*aEÉǍ?uEKî{ØB?b*aEÉǍ?ïøj"Ä·;?CÎ=€qĖ?NWtqýâ6?CÎ=€qĖ?ï®êWæàŽ?'N"QÆ·®?"Ej
's?'N"QÆ·®?ïÖ¿$¡'¶?y´§Îxæ÷?t m›~i?y´§Îxæ÷?ï/~~¶?Ž¥ËǍI‰?šð''7?Ž¥ËǍI‰AGN4FGL J0640.8+2432?ÒՉ±'f@!~O3Cú+À; C÷¦•+À<r2ËŸ@!^Î¥?=?÷"]wª[‰?πl÷м?ׇS±Wü@@ÅEÅ@Ìÿ¹^0¿ïþ›A9†?ïÿöµš?d-o¶•h?ȯD;CM¿Ü\O™-
¿í1}‡ AGNbcuRGB J0640+245B?ïý*~"ì?1HÍ-U²¿?6¬
/¼Ú´?1HÍ-U²¿?ïÛÁ!Ñi?wæL´i?ro
ád?wæL´i?ïOªCØ?"Ÿ&UH??–½ÌoRö?"Ÿ&UH??ïæûÑ`ôü?WVW" ?i.§JÅ?WVW" ?ïüßtͺç?9ääÀuîW?9W‹0—Ï?9ääÀuîW?ï9w‰¾"?¦yùþú•Š?˜ÑÍc¥¶?¦yùþú•Š?ŒŒŽ?Š¢-va¯h?‰Yœê·?Š¢-va¯h?ïªr9$Ü%?z¥
¦ëÁw?…cq¬z"Ú?z¥
¦ëÁwAGN4FGL J0641.7-0320?Ø?nù:œ'À
oZÎÀ8mô¡',•À;%ºÜ	€²@Îü<Ñí@nòÇ2Y?°—Uq¡'ò?Åß_vˆš@L{‰
Z\@ƒs¢¹ÿ¿ÑyÁ¢w8Ç¿ä,0àrœ¿çG–,&Ïx¿ëymª'†¿ïy?n)ÿ¿ïû!sîfAGNFSRQ3FGL J0641.8-0319PMN J0641-0320?ï엦Wö•?`oòãrc?chYåâc?`oòãrc?ïé²²ÞþÂ?tö\Ab3›?fMLß¾?tö\Ab3›?îèëc2KÏ?—Ù²:.·ê?¡qIÉk§?—Ù²:.·ê?ïúÿ'q?1ü'YB,·?DÀ›*6?1ü'YB,·?ïãþKí5Å?gßn("V3?l³ÙÊú?gßn("V3?ï>$¢e‰á?ªÄò¨rˆ/?˜;k®'YÜ?ªÄò¨rˆ/?íéN†±ñ?£+7bÙT?°µ‹Êþ?£+7bÙT?ïä†YöÁh?^4Í'í°?ky¦1ß?^4Í'í°AGN4FGL J0643.2-5356?ê-ñðÀ6É/Ÿ¾wÀ:m÷hÉ™À<qދ;2@ÊkÃr†@"NÿA"?½>™~ýÈ)?'I©¹™¶—?ÓÿZS2¬û@\r˜£ÐT¿ã[m¯0Ô¿ãr2aüõ4¿ã£ð4°áµ¿äžh5s¿ë#î¼á>¿ïÿ÷1$e:AGNbcu3FGL J0643.4-5358PMN J0643-5358?ïýúŒgq?*ºBñz¾`?7@*#/<?*ºBñz¾`?ï÷‡Á9,?QíHl§/q?PñØzÍø?QíHl§/q?ïã'@Éb¤?m-(ÃÙä?ln¿ZYKû?m-(ÃÙä?ïÿ-øê?­?‡™–µ?@ÜåPD?‡™–µ?ïü™ykÚL?5žkÿ¦?;43'™L?5žkÿ¦?ïÞ4-%Ÿn?}Þú9S#?på鄍 Á?}Þú9S#?ïÚr$4½¢?}>±mU*ð?rÆííà??}>±mU*ð?ïýÏ#f?%
c!ˆ?1‡eEDNÚ?%
c!ˆAGN4FGL J0643.3+0857¿ï•y~ª@Jf:Ç|+À8Eöx—ÁRÀ;w…@˜Cz~ l@ê#ÚЛŽ?ªeŒÄ'?Æ¡°êC*L@g:6\³_@žS;¿Õd¾{PX]¿à¤¥0¦ù¿çPáïɧ¿èó­aL¡¿ëlb©Ã]¿ïÿ†}³	,AGNfsrq3FGL J0643.2+0859PMN J0643+0857?ïËÁ£]µ?ˆ+ÛH?zw¹ÿÑk?ˆ+ÛH?ïÁ´4œâ?‰@«ÊQP?%å¿Mb}?‰@«ÊQP?î]m­Ç<Ú? G‰Q?ª)%$hc? G‰Q?ïóDDÊ×¢?GW,\ÑÁß?Ywv©‰Œ•?GW,\ÑÁß?ïO¶ì»ª'?'e6Äõä?–	"ccCö?'e6Äõä?íÃ[±ƒ~?¼-·%ú?±å"xË?¼-·%ú?ëÕaœZǪ?¬>ñ»ñ<¬?ÀªyŽ"áW?¬>ñ»ñ<¬?íbæÌ?z)ž¨'Ü?Š˜D®%"Ù?z)ž¨'ÜAGN4FGL J0644.4-6712?Þê'	°À9‡ºùe²À8½CwN7À;̾&@Ü@œrêƒA@K²™ß:?¥ìAº¾
?¶ïôAðe@ì-BXj$@¾&-f?¥?Ù:!¹ä¿Ûn¤éb/¿âV<»È¿á½4ßݵ¿æTd ;ë¿í»Šàn?NAGNfsrq3FGL J0644.3-6713PKS 0644-671?ïû×Ôè¥?7¿óŒBc?@ «_nÝÂ?7¿óŒBc?ïõ:÷€]?[¡òv/'O?UɊ>U~?[¡òv/'O?ïÍHQõ¸v?€úà@ÿòè?y[Öùu+?€úà@ÿòè?ïÿä¢èˆü>ࢆr'».>ë]à'uN>ࢆr'».?ïýô!ûÖ?'µ"VpƒF?0^øæ:vÆ?'µ"VpƒF?ïÕZgª‰+?€íÃE>é?uRÌ¾Š?€íÃE>é?ïÍÝ£´¥?"˜ó·?y.ohÎ?"˜ó·?ïÿÛû=ù`>酊œÙg'>òCÌßâý>酊œÙg'AGN4FGL J0644.6+6039¿à \›%N³@6ÔÇm{À:_þKÊÙ®À<'©1½n@'²'
@a× åÂ?»c òÏý?–ÇùB:{ì?à<í'hr°@Z]ÿ—¸?ïøC""~¿êxdàTi¿áZÕ¤ãc¿×ðŒma,¿àШ# 9¿ãzˆ\ZsêAGNbll3FGL J0644.6+6035NVSS J064435+603849?ïþh²­?¶—yeü?);;ø€ñ?¶—yeü?ïôù&›9?UÅ»J–>­?V
ÅMX?UÅ»J–>­?ïùO­oí×?Tðãäº?JÁJ^…2æ?Tðãäº?ïý;äÿëÕ?ÍÞ»r	½?6 שÄÎz?ÍÞ»r	½?ïþ1U¯×@?"¿vÒȵ†?,ê¡"ɑ2?"¿vÒȵ†?ïÖ^tæ˜?voT{Ì7?týP½M¤?voT{Ì7?ïùѓ8µ?b[AÓâ¦5?H¹³…²?b[AÓâ¦5?ïúµ†gÁ8?2ð•†KË?E)æÉûü`?2ð•†KËAGN4FGL J0644.6-2853?î«£K7û‰À,&o"5ÒJÀ:Í»DLÊÀ<iŽ2]J^@ Ó ñ§£?ùdM‡rO©?ʈBZ¨m?ҁþÝÁ×@	bçcQ0@
hs[í¿ïÿ› 'V‡?ïó¯ûî|?ÀEýz¿ŽÌ¿Û'@5пÏ	IÕ·4¿æ²d ï&AGNbcu3FGL J0644.6-2853NVSS J064443-285116?ïòpb"ž?TÙÖM£Ö?[:ZR\?TÙÖM£Ö?ïÞYày°y?ƒ' {"‰~?pÓʶçš?ƒ' {"‰~?ï¨
JHŠ?€2*Å\ˆE?…ý7¼±?€2*Å\ˆE?ïÍSŒÑ¾?bˆá´ê¿?yVr†?bˆá´ê¿?ïá#.`ï?h['òîa?nÜѽM"?h['òîa?ïwü !ˆ'?›7.Ñêê?'|®%Û?›7.Ñêê?îÐ÷1`ÿ?™Hœ¸F?¢ðë2"?™Hœ¸F?ïåŸEnä?Œ¾½¨]%?£LšUˆ?Œ¾½¨]%AGN4FGL J0646.7-3913¿í›_Ç»ÀáÀ1›ÜY1Ê}À:JiýʛšÀ<HÄdH~õ@–ìËÅ»¶@wdã¯ga?Ä:DŸlAr?¯'ªa4oÁ?ãzksù@	‹–ßU§¿â§´«å¿ç¼¯ŒwG¿ìc1" Õ¿è«k…L¿ïþrÎ\¿é¡–R½<6AGNfsrq3FGL J0645.9-3914PKS 0644-390?ïþU_FÑ:?)/_5BÈ?*ªøž'†?)/_5BÈ?ïõŽ95£?Xmª(6C?Tãn>'R?Xmª(6C?ïÄ#÷½!š?"¿,""#?}îC^±?"¿,""#?ïûįFÿï?-š¢¬ûØ	?@íBJùq?-š¢¬ûØ	?ïþÝD?5yCƒõ¨?.Îꋏ͓?5yCƒõ¨?ïٙqß?€¥ˆ6"T?s3G?‹?€¥ˆ6"T?ïËDßX?'*)-z©?zq]¢1íˆ?'*)-z©?ïà#5ƒ?bZb¬‹û?oÜúøETÖ?bZb¬‹ûAGN4FGL J0647.0-5138¿îi¸qåºHÀ5—Ø'sâPÀ;•YÀ<¥øZQ
@!CŽqwÛ?ú7ZYè©¢?ÏÌt7_gÅ?Âm9©Äßî?óTsۍ@­Ô€Jh.¿çX-ˆÏFû?ï‰ü¾, ¿åþ‹#¼H?Ò$Œý)¿ä6Ÿ™Û¿ÐÛPž(­AGNbcu3FGL J0647.0-51341ES 0646-515?ïÿ'g J£>ÿÜS'z5ï?f3­CÚ>ÿÜS'z5ï?ïõÂj?Wë{›ý+?Uóþ6s¦ã?Wë{›ý+?ïõcÚEn?Eºæ]°Ô¸?U8K†sD™?Eºæ]°Ô¸?ïüa.2Q?%!2K»[w?<öŒcUå˜?%!2K»[w?ïÿlƒç½?
<vQ÷C?~óøx?
<vQ÷C?ï×aœ§?ƒØW6t
Ÿ?tÏAô«?ƒØW6t
Ÿ?ïí1%‰Há?m¸Û(F7?bÎÚM{ÏR?m¸Û(F7?ïõÃÎ\«?JÌZ³OÀÊ?Uâx<Ë
?JÌZ³OÀÊAGN4FGL J0647.7-4418¿æ^
uÀ33sâOëÑÀ:Ãf½ÌÀ<"ERðgÝ@Òÿ+ní@='¯š?È\S}€‰R?ËW\È­ÙB@·kÜÇì"@äNs«s?äšF½©™A¿ÜùÀGƒL¿ä¢­>'¿×˜Wš¿ëé¡éÛÑ¿ïÿý{ÁA~AGNbcu3FGL J0647.1-4415SUMSS J064744-441946?ïÊÏç´Y¹?uа¹ö M?z˜F|?uа¹ö M?ïéÌʞtJ?aHž'B[q?f35*'öx?aHž'B[q?ï"?D/ý?€aöÕF?Šð.í!'¼?€aöÕF?ï«+•£ö?bŠäþÒms?…5­Å?bŠäþÒms?ï&?â:"ž?˜I¿YÆ?›8°fQ?˜I¿YÆ?ﰒɾü?ƒá­Y"ñ¿?ƒÛM™güÞ?ƒá­Y"ñ¿?îD_Ÿ)«?œûõ3'6u?«º
ÉO?œûõ3'6u?îjœ^£'?ÓßÄ(ìç?©V:Í?ÓßÄ(ìçAGN4FGL J0647.7-6058?èvÇ¢kzLÀ7ï´_½ŒÀ9ÆöÞN«À<R«ÿÍ«@ g-Å`@Wç^j?³(¤9Ù?¥ÐKÉt?ñà^åh¥@ו9?Â(mÀοæ8éU™¿ænÖâÐDQ¿ãIŠ"-Qr¿í7!ŸŒø¡¿ÑH¹­5WÑAGNbll3FGL J0647.6-6058PMN J0647-6058?ïý°ª'J?"€`"šo?2zª¢»"¼?"€`"šo?ï÷YË^Ÿ?VÞ¯¡6|¯?QáLqÒE?VÞ¯¡6|¯?ïìREÄ?Z'$ âýÕ?c­ºôï;ô?Z'$ âýÕ?ïÿÃûG?üõ4ƒs?g¤±Ž¶)?üõ4ƒs?ïýŸ¼ãœ?-"``ý%?3ÒÖÁÒ?-"``ý%?ïߺU›­?or1eE±'?p"ô·¥…Ï?or1eE±'?ïç"ãBô¶?vð†»õ|Ø?h{õdá£?vð†»õ|Ø?ïý©A¾w†?+%Œ·Ìö?2µòéDJñ?+%Œ·ÌöAGN4FGL J0647.8+4527?ã8ôœä@¡@2_–لÀ9ÏÒ␃pÀ<žßS¸@"mðÉVK@/»õäô?»ïj0 [Ö?º®?-÷?øäӛ'@¿ü¯¾¿W…ï(þb,¿åýÞó?þ¿ë4úqK¿éªBÿY¿áÑCõ"Vl¿ïÿçáüúAGNbcuB3 0644+454?ïô

ðÉ×?WÌÎ=zàÍ?Wëéõ1ñ?WÌÎ=zàÍ?ï×Z"œsO?}&"?ÅÄA?tRT?}&"?ÅÄA?ï'cÆè¡?ŠÛM0Cñ?gBh#c?ŠÛM0Cñ?ﴑ8i'?iŠjqùő?'Û±ð¿!"?iŠjqùő?ï²bÃ,ë?†šZÅÚ{r?ƒgO+¯H?†šZÅÚ{r?îâ¢Üú?©ÆJŒøÏ?¡ÕÞ3—X?©ÆJŒøÏ?îö»Þ'ó?¡³²pj?®P"A:éÓ?¡³²pj?ìÖ*cMNµ?¥•öÆÍ,º?¹N¬ä¹£[?¥•öÆÍ,ºAGN4FGL J0648.0-3045¿Éˆ¶Ä[À,M‰ÎJ{NÀ9^íÌ ÕÀ;öJ…_Oò@/"⥧@tÁrüw?ªc;
Ȭ?À¢½¯£q@lN¡MÃ@.y¥ˆe??Û¡Ñ@ÏÓè¿àXR§lÀó¿èl3/u¿ç2,ئã¿çØì`¿ïÿî' ÇAGNfsrq3FGL J0648.1-3045PKS 0646-306?ïüêÿ4J'?2Ž?αs¯?8¨ ^"ä?2Ž?αs¯?ïôá+²?\ø
'UÖY?V=¨Ic4þ?\ø
'UÖY?ïÞé·ê¬?fVõŠÿ'?p‹$ D½Ð?fVõŠÿ'?ïÿ9´~*?	Ò½}+õî?ÏÏñÅ
Ð?	Ò½}+õî?ïþk"!‡?%¨'I"×n?)FÐWq…?%¨'I"×n?ïÔËj:ö?{jYú˜,?uü9´y?{jYú˜,?ï¿]…c¤?'YÀÝ š˜?€(ž©Ö­?'YÀÝ š˜?ïýì3¼½X?#îÇþ
0?0žbˆÃ5?#îÇþ
0AGN4FGL J0648.1+1605¿îì˜ú.Ò@9GüÀ:îÓr&ŽÀ<cp'Iü@!Cö6D5?ûËh´€?Ë5ª†ÑÀÒ?ÃKé¸jë?÷!iÝl@š£Š3J/?æÌ0$ŠùÄ¿ïžQYŽç?ïþ"Õ½6W¿à•NEÞ0¢¿ç榒¦`¿	ã‡AGNbcu3FGL J0648.1+16061RXS J064814.1+160708?ïý½gÛ?&@ÊR?27ýH'o?&@ÊR?ïâA®ÿö?sŠ4éðà?m¾QÏáÉ?sŠ4éðà?ïè·B»«+?p¤¢¢†ò?gH½(×ôû?p¤¢¢†ò?ﻕ ÷Ã?mšÔͺB?—Â?Ê?mšÔͺB?ïùÍÍd£?@™bé	"…?HÈÊ%©åô?@™bé	"…?ïGZÒI?¢'~ŒØ?—¾œn×?¢'~ŒØ?ï¿s$‡@H?'2…ðŽ­¶?€#6Ù`z?'2…ðŽ­¶?ï_]Ëj?†oË1D°.?"ÔW‡Z»?†oË1D°.AGN4FGL J0648.2+1745¿Õ
ÊJˆÜª@MþûôÅÀ:ð‰¹QÅÅÀ<]vâµl^@ ݁ñ\N5@¼râv?Á=èƒažÖ¿´Ã$¹ô?òÛ>µGu
@1ùeÜþž?luS¿ç
'àÂÍð¿çeþj~¤¿ÛA"YÁg¿àyVbã$'¿å®éŒöóèAGNbcu3FGL J0647.8+1751GB6 J0648+1749?ïü"m°?,üÂ"?;ß-]P?,üÂ"?ïãÙÛAô[?lG+ÄD4-?l&$·,m?lG+ÄD4-?ïõ}Ip¦?TîËÈ<¸?Ulõxqê?TîËÈ<¸?ïé衔Å?K¯¸ÓB$ú?f^N"ƒ¤?K¯¸ÓB$ú?ïútWë¤S?;ßÉ¿ð•u?F. ßDø2?;ßÉ¿ð•u?ï%i_†è?£Hʁëhs?›RÝŸ‡?£Hʁëhs?ïú·gñè?RPÑ;ô.?G¡"ä¶??RPÑ;ô.?ïPè™m5?…Q"rB{?•âì׀Æ>?…Q"rB{AGN4FGL J0648.4-1743¿åNÓ¿§—«À!=‡rO¨µÀ8:êh¿;À;7SåZbL@ªšhÌr4@í"Zm3à?¥Ñl»?Ào>|<'@ãxt†@*‰
tx¿×Uˆà%¿â×nc¨¿åîŸ	›	¿æîQ Ü"¿ë1ÓíR~R¿æ"% ËÒ|AGNfsrq3FGL J0648.8-1740TXS 0646-176?ïóû-™|z?{^ž(ð?X	¤FV]¨?{^ž(ð?ïê)½FO£?r}"Þ>ë?eÖB5?r}"Þ>ë?ï¢VÍIÒå?…©êPsé?‡jL¾¹R‹?…©êPsé?ïÿpYHy?®=¶9ý?þ÷U‰z?®=¶9ý?ïï䬒o¯?cà1
ëg¬?`Sq¯ÙA?cà1
ëg¬?ïgsüžn?ªz‰wÒ8`?"€h¢'?ªz‰wÒ8`?ï4g:̯œ?–¤ÈjË!'?™s¢úp"?–¤ÈjË!'?ïýÙé&/ü?'ƝÓòà?10µ1‹A?'ƝÓòàAGN4FGL J0648.4-6941¿èbI!ÆFÀ9'h›Œ¹À;×5>¦À<üF€íÑ)@!M˜.‹?ü°åEi–?Óñž"S"?ÂwOWV(+?òeR…?ù(Øç7\8¿ïÑ£Ì"'â?ÊUÆ[ªq?ïՄ̂úò¿å']džg¿·ò'ÿNTL¿âù¡A-ǹAGNbcu1RXS J064850.3-694519?ïÿÿDÕX?ˆãa%/?ÀD$€ì?ˆãa%/?ïñ1*ÅP'?^I¶Hü(?]ªTb¼è?^I¶Hü(?ïâÝl¤e?iÝ=4Í=?m""|kÚÈ?iÝ=4Í=?ïï±%€(?Nô]÷qí'?`Nþ™ç/ï?Nô]÷qí'?ïüMϧٴ?@ÈùGH?='5_^f?@ÈùGH?ïÈVßX?€|qêx?{Ôðpªd?€|qêx?ïÎ?…ì?{לÔu"Z?xà="vtE?{לÔu"Z?ï»Cº–?xÛ¼w"´÷?/:'¼ro?xÛ¼w"´÷AGN4FGL J0648.7+1516¿ßz0GÆh/@KÆ!·à¬À8Û
LŠNÀ;ž¡[.ú¿@!³R)˜?ú¿gJ¹?¨Ã¤¯ø*Ê?¡œbY¯ý?÷¢™Øƒº4@ ΁­¿–?íók›Æp?¯H\æ
¿ÙςŸ,*«¿Ñâ"~ea¿ÚfÝD>He¿ÚI"ÇȁAGNbll3FGL J0648.8+1516RX J0648.7+1516?ïþ'xìXŒ?ïe÷'¤¨?&èoõ©Í?ïe÷'¤¨?ïêV˜+õ?t†ÜD[?eê©D?t†ÜD[?ïæ*D¢?x4gfǯ?iïÕÉTz?x4gfǯ?ïî_ýt=?MûdëýŒ?a §?Ñ?MûdëýŒ?ïü
?7»ßx Ò??ǗK:W?7»ßx Ò?ïG'Yù	…?¡W€õ|Ò
?—
´½o3U?¡W€õ|Ò
?ïè-Šõx?ut•¨Ç'¨?gÒuV Z?ut•¨Ç'¨?ïâÃ7çfÆ?]µÙã?m<ÇÙ`jŒ?]µÙãAGN4FGL J0649.3+2230¿åCLâB,@#<yÔØ4	À;&oþDÀ<~+qÒ
@ ×´?˜?þ·.ÕÖ`Ê?É¡Ä
†k¿?œ?÷Wó?Ì6sCš@8Jaοï{KeY -?ïþ"åÞÊ¿Ýû'¾Šêª¿á$"…|+¿ç…Õ"ܤ¿ÉýC¸¨AGNbcuGB6 J0649+2228?ïþÚEÜ-=?Vrd6˜ý?"[ž*Õé:?Vrd6˜ý?ïï²@?d3ÞR%ÿ¨?`ýM뿯ï?d3ÞR%ÿ¨?ïó\½†x?Mž¤ã±íå?YGܒ±€¾?Mž¤ã±íå?ïõޙR÷Ê??´í4îP:?TBÌÓ_½p??´í4îP:?ïþJѾà?*1mô[<Æ?+Rç7˜í?*1mô[<Æ?ïˆÏäH-Z?•G>ËYÃ?Ìíô©y?•G>ËYÃ?ïêqLë¸m?pé1sËÂÌ?eŽ³5CÓ?pé1sËÂÌ?ïÚ]n›A?d‡£ùÏ?rÑHÓrŸ*?d‡£ùÏAGN4FGL J0649.5-3139¿í¿ïY>µÀ,k-M@$³À9þˆˆ˜ÀÀ<!V˜"	]@!«ÝˆÜ²ô?÷½w$#Ë·?Á=wš@]"?Ĩԟÿå(@©)Äõg÷@	«èCZH¿ç¼ dŽõÒ¿éÛiQ;¿ß[™C]wÕ¿·ùl'ûDÚ¿×ÙÖà÷Ò	¿Õ^ŠD<
AGNbll3FGL J0649.6-3138NVSS J064933-313917?ïþ8wHZ?&ëŒMÛþ¿?,xžÅÀ?&ëŒMÛþ¿?ïô;"ç¿S?]s!¯ƒ?WˆÖ"v3?]s!¯ƒ?ïðæÚ¿ÿŠ?P ñq,Í?^2JLé?P ñq,Í?ïûtgÛÜ_?-?£qpBü?B.`͔_ˆ?-?£qpBü?ïý1{o"j?2C¿Ý±ª?6t#Č
[?2C¿Ý±ª?ïÓåpî»Æ?†ã'(e?v
Gky?†ã'(e?ï͉úüF?|5ëŸJÞ?ys:èdÕ?|5ëŸJÞ?ïï¨VǞ?S• í7?`Wø´7!Ñ?S• í7AGN4FGL J0650.2-1636?¸yQD1CÀî軶$À9"†AΩÀ;s•}@'/bn4;@¿~/°È?´…¢ì©Œ?¨›'Ÿgu?ò=ÂÙ.@
ï+E((=?ïèsAI¿à?Ä UàÝ¿éAΡ¹"̿塏Òpz¼¿ìÁr%·¿àÐ%FáeáAGNbcu3FGL J0650.4-1636PKS 0648-16?ïÈøJ¼æ?°ìŠ±üP?{ƒÚêÕ?°ìŠ±üP?ïòzÉþCñ?[''"ì'J?[
k…?[''"ì'J?ï¯6³+'?"ò÷SÀ
Ð?"2{Ø\…¹?"ò÷SÀ
Ð?ïò%ÔGaá?G…Ý€ZI?[´W~ú®s?G…Ý€ZI?ïÛn‰v?ul'Sôü›?r~ȵIy?ul'Sôü›?ïÌ¥aÆ;?ˆɽd)>?y­OuaË?ˆɽd)>?ï/W®4'Ç?•:(ô)­Ú?š
0ä$?•:(ô)­Ú?ïÅyžsëW?nÏH/>Ê?}C0äöЇ?nÏH/>ÊAGN4FGL J0650.5-2851?ïCóÑ.ÂqÀ)ÌE˼+•À:³D…klÀ<7äæŸê@¨Ïqí®@¯äë8?Ïœí¡ƒÚ?ÙX«þ +ï@$ÚZT	m@
™á*Qã"¿Î) zb¿æ}ÿ	_û¿è@›f"sÈ¿åýŒBn¦¿ïüA&PÍ¿ðAGNbcuPMN J0650-2849?ïñ[ü¢u?WÜ)†ÛØ?]÷Gå¾Ö€?WÜ)†ÛØ?ïç­&ü?g‹Þh­¹?hRÙ×¥U~?g‹Þh­¹?ïS[¼ê+­?ˆ•¬³l?•"ˆ_JîZ?ˆ•¬³l?ïÏ×Z礌?Z²™T®7Ë?xRk1z??Z²™T®7Ë?ïøsóÜtú?Q¥'Ãn?N00ùì£0?Q¥'Ãn?õ£ŽC?'Ÿh¹È{>?ŠšÂ¤ÚßB?'Ÿh¹È{>?îòûG?—+· }? ÐKŒRÀ?—+· }?íôÀ*æ€?™Í†õÁÒb?°Yÿ>:؁?™Í†õÁÒbAGN4FGL J0650.7+2503¿ËÍXÁjÍ@&áõ±ÈÀ7ËUúÞXÀ;$ö%‹«@U)[™ñ?úãEš>H?›QZ™1G~?Hõ<WŸ#@m|²F@~Ÿvþ9¿"Ô#ƒ<àÜ¿È"HJ¸á¿Ûúœ~Pg÷¿Ô'")Dó¿ÞÇýM´¿ÈJì¢ÖWAGNbll3FGL J0650.7+25031ES 0647+250?ïþÓVöÿ?î"FòŒÎ?"ʍÐ^6ø?î"FòŒÎ?ïîÙ=?jœ‹{ȝ?a€ýeûÃ??jœ‹{ȝ?ïÙ¼»Ìc4?{*ní{Ë?s!¢9jͱ?{*ní{Ë?ïÿq›‰ïê?VøPåo)?̏T­j?VøPåo)?ïýô¹"¥ƒ?(cÏuX"ª?0Z1OuÒç?(cÏuX"ª?ïŠ×uƒuý?–*­•´cž?J"¢'À?–*­•´cž?ïâœÇbb?v¼ü‹?mc8à}²?v¼ü‹?ïÿC¤fô?^Ë;?‡ªg©?^Ë;AGN4FGL J0651.0+4013?ïÿÿ£¡@1Å!Ý À9ÖâӟNåÀ<Q¹¾Ó@J
ÒüfÃ@?¦›à›·?µc¢áy­?­âDc\œ?öf
{ÅÕ@ë÷/ü¿ÞÎAìßg¿à>ÌÄiQ¿à1ZJÏ1+¿àõ·§¡š¿â¡5íËJ¿çÒtvÊa¹AGNbcu3FGL J0651.3+4014RX J0651.0+4013?ïûýÅpÀ?=ný;~n|?@ë*|X7?=ný;~n|?ïïÓN¾vj?^ô›?`,±uÃ¥?^ô›?ïõ[€üŒ%?a/óA¼r?UHýî*‡?a/óA¼r?ïâü×ÑÒ?Qé­h<W?mè*íݝ?Qé­h<W?ï÷WÌn?EՁxOw?QPhô¤#?EՁxOw?ïºëßó¬F?"ÌvjßT¶?EùÍü˜?"ÌvjßT¶?ïáñéfá?z…VB?nç¹æ©?z…VB?äAL?uƒ5µ¸?ŠÐùظÎ?uƒ5µ¸AGN4FGL J0651.4+6525?é%¡XfÑ@8ñ"<:CÀ:Zys‰d˜À<²®{¨íÊ@©µß†?þ±fYÑ,®?¿S>ìNó-?Ãb;ÉÚª@qÕ"äF@CP³¡­¿Ý
™E彿ãvõÊò×ù¿×L*ZÇvͿڝDÿŽk¿é
jKÎ4¬¿ïÈ<¿2ÛAGNbcu3FGL J0650.9+6524NVSS J065125+652458?ïõ>˜ÂE?X¡0ø^Œ?U'ÎÄf(?X¡0ø^Œ?ïëPKz…`?e5nBô{?d¯´k]˜K?e5nBô{?ïÜ¥¼iç?nÆyôP0?q­!®Ìì¸?nÆyôP0?ï©týOn?g^Š¾ÑÆ?…¸¢Êúøu?g^Š¾ÑÆ?ï&s'aLT?™NL§9?›1«?o"?™NL§9?ï½°âWðÏ?€‹yõÁ7?€"ÇZŽJ?€‹yõÁ7?î‡Àæå|Ç? Çð³ËÌ?§ƒñ•ό? Çð³ËÌ?µŽ?‹¬ˆÏ?¤ä"«Ójç?‹¬ˆÏAGN4FGL J0651.5+7956¿äªjÍ(g@:®ÿ:Þ"`À;/Nbc¢gÀ<šz¿ÖD@ÌvŒyK@¶ÌD琝?À0D
û¿Äà7bÂÂÞ@¿*?nªÙ?ñÕ;0W·¿ì/AT©P¿És—ý7MÊ¿àQ½e¿ê˜YþyC¿Æ)£L¿ðAGNbcuWN B0643.2+7959?î§ú*'?ÄGe®@×?¥Žp`Y>Ý?ÄGe®@×?æU\~c»Å?˲
Ý¡í?ÓUG8ˆv?˲
Ý¡í?í¯âQª}Ô?¢z[cC•X?²€íqb6å?¢z[cC•X?îùÎo†˜?"3eÐAá? c–ç?"3eÐAá?ïVLs²:‹?¢î¢ùSc`?•6q'O´"?¢î¢ùSc`?Á?Æòöµ²?ÁÿÂw;ÿ?ë°CBR"?ÁÿÂw;ÿ?ì<À? ©Ù?§ø÷^W	?¾þú±7?§ø÷^W	?Ù#þØÆã?È£@}YÙ ?ãn"ùœ?È£@}YÙ MIXED4FGL J0652.1-4813?îýŠÍMüÀ3ÃäÿÉy[À;	¼AdNÀ<³""Æ@ 4'éª?þiÀ=rQV?ÎÜ垪Ð?Àÿ±%§Yv?ñð*Ÿæ»@Z²~?ï'usI£¸¿égý	«zm¿Þ?M]Uñy¿áïç"7Ý¿ßPcÛÅ¿ãΰœë]²AGNbcu3FGL J0652.0-48081RXS J065201.0-480858?ïþ•a¦Ž?À¨¸hFä?&©åºMG??À¨¸hFä?ïõ¸8®1?TTɽB%?T%Üne?TTɽB%?ïðæŒÚU?jî©vÊw^?^3ËQ&	?jî©vÊw^?ïö;mê>M?4*I–¼Ì?S‰$A€æ^?4*I–¼Ì?ïýÏp
Å?/ãœí?1"¡Å‹?/ãœí?ïكe¿fL?€%Zñ%ç,?s>M,«r?€%Zñ%ç,?ïô'Éaw-?d;>TW{?W°lõ™Æ?d;>TW{?ïؙÇfÜX?`¡ˆ/̼Ö?s³Mñ«ü?`¡ˆ/̼ÖAGN4FGL J0652.5+1932?çÁTœm.@"	j­À:€ÈlüÀ<&D‰œÌT@jßÃ@zÓ}Àõÿ?פ˜Æ5?ߊë¡#P½@¡~4¹E1@ñ'1ó9?ïû	öùÇ?ĐK<>u¿âÛYWŠ¿ë¶¹ÐpÆ<¿ïւäY±¿ïÿ§ëkôEAGNbcuMG2 J065230+1934?ïePC[Á¿?'.³´²U¦?"U÷'Ïú?'.³´²U¦?ít¹ÖK?µ—b¦3?´_"0á²(?µ—b¦3?íV·¬Õ
´?žà&«A?µJB˜{Ãb?žà&«A?ëéó›m¯?š<,.›Ä£?ÀYˆ1'IC?š<,.›Ä£?ê‡bÕÊ\?¿ŒÎ€½:ð?Åât«ð֏?¿ŒÎ€½:ð?à×¢³ôŽ³?Ñ+òòPj?ÞPº˜â›?Ñ+òòPj?çP÷ášÝ?³¯ìG*?Ðý^<ÊG?³¯ìG*?àˆ'‰åO?³¨%0bµ?ßÎï°ì5b?³¨%0bµAGN4FGL J0653.6+1636¿íÀd^ßÍ@Û2‹m†ìÀ:(°ÿèÀ<7ÚH¶R7@–¼f@kÈ:–ÔÃ?¼= IŒ¿5óT|'Q@äO¤XŠ¿ã"¿"g¿æ(þ¦ä†¿ä_¯""e¿ã³Š§ß­¿áa{_ò®ß¿Ýé¯Ü|SAGNbcu2MASX J06533986+1636432?ïî&œªxÃ?—^Õ°ä?aÙc\fud?—^Õ°ä?ïîTÎRLÃ?i÷žÃ^=ë?a«1›ÕEY?i÷žÃ^=ë?ïéBp+ÐØ?oÄxËóÓ?f½'§–?oÄxËóÓ?ï÷ö&ûí?7ї"ÙO
?Púȱ ?7ї"ÙO
?ïí\Ö´pú?X=Íë+ÄÁ?b£)O®Í?X=Íë+ÄÁ?ïyP%²A0?œ™áqTf?ÕûA Ô?œ™áqTf?ïåCç"?wE0'8f??j¼š¹¨Ð?wE0'8f??ïÛã…m_ ?aΩbcÉ:?r=V^ó·?aΩbcÉ:AGN4FGL J0653.7+2815?ãCïX'é&@)ÚÑÐAÌSÀ:7zÀ~hÀ<U	Ĥà@G_ÏÉVv?üê"Ash?¾È"™"‰?Ðk/coæî@®þ#†î@#óï{x¿èÉà>¿j?°r@þç•ë¿Ò¾¶4žm¿Ø'=4p¿çä&Eüd¿ïþΈ°=AGNbll3FGL J0653.6+2817GB6 J0653+2816?î[åsY5s?¨j³F?ªA¨ÆýØ?¨j³F?îvo£ÚmÓ?©öaù°‹?¨™ÂY"Ó?©öaù°‹?îÒáŸþÊ?ì½£'ý?®ÂÑæÛúd?ì½£'ý?î¡é_];M?FS™(´@?¥ájÀ+?FS™(´@?ç9›Zl«?Řõ•ÿí?ьÉK&Þ«?Řõ•ÿí?åÎ9Ø؍?ÐJÂû"ê?ÔcŒNNäâ?ÐJÂû"ê?ä~øR®ðæ?¸ƒµì0v]?×Z¢4?¸ƒµì0v]?èdAƒ¶‹ö?¬É÷Ö÷Ú(?Înùñ%Ð'?¬É÷Ö÷Ú(AGN4FGL J0654.0-4152?íÃ=VøŠ@À1BjDAxpÀ;%ð†æ8¯À<"ľá@ ´£¶(@å¹}d¯­?ÄóSIS0¿¦	6õh?ãC
€òç@ƒ		i
?ïcÐT@Éõ¿åÖCŒ¿è"Î1&¿Ó–[@î\¿¿á¦R_Hdô¿×V%Pœ{AGNbcuLEDA 571171?ïî
Ç[Ê?¡1O}Ö??aòäg¦€?¡1O}Ö??ïõ¥
»ñ?WrúùyáÀ?Uòµ®þñ?WrúùyáÀ?ï÷l)Ai?C"B$ç7×?Q'®{n,y?C"B$ç7×?ïûkÌôó?&­úG탦?BPÏíí?&­úG탦?ïþÛQ8Ç?'ëióG6?.KՌIR?'ëióG6?ïØìÝ'QÂ?w'%§èe|?s‰'|%R½?w'%§èe|?ïùoÖZGÓ?^ÿƒ$*‹S?J@¦ßþËA?^ÿƒ$*‹S?ïçsWÌ«Ñ?Z{w•ÆÏÕ?hŒ¨؏P?Z{w•ÆÏÕAGN4FGL J0654.3+0923¿èét$Y@—ÊÂ0'˜À:¹C•%À<:̂úñ£@ 	Ip·M4@Úÿ•võ?Ä2T"Œó?'NÓLè?ÐA
œÛ¾@"²4°·?îQ.ƼèS?¡êˆtƒ4¨¿å
!AN¿â£¹þ"ï6¿ÚG5ß
&¿æ˜ˆAØg‹AGNbcu3FGL J0654.5+0926GB6 J0654+0925?ïê¤tá?½~nß }Ó?Œ[èӕ?½~nß }Ó?ïé/ÙXî¦?rkµé¯ÿ0?fÐ&€•º.?rkµé¯ÿ0?ïôz7ˆ!?eˆ¥&$âÏ?W'ï,Nb?eˆ¥&$âÏ?ïú´"ÿ*å?)1Ç؝þ?E/tÞ§`?)1Ç؝þ?ïüö|.àÏ?5BÒÏy‡!?8LôZ»?5BÒÏy‡!?ïhúýá?Ÿ`WN]•Ž?'ïÀ™mã?Ÿ`WN]•Ž?ïó/€åÝ?p_¢I?YÕ¡/®¥
?p_¢I?ïìƒfQm±?T=|+Wn<?c|™–P?T=|+Wn<AGN4FGL J0654.3+5042¿å×%͈Î4@5ˆ‡"žÀ9qal+¢À<Ë­b@ê/o¯:k@™'¥R?¦æÏ=¦Ý?´%`Gú|@2Ÿà·ö@ð…×ÅÏ-¿Öü°?Mrпßv–_Ruï¿ãšÑ!Æ#e¿â³9žeË¿å«äT¨ÎÁ¿ïÿäQMÐmAGNfsrq3FGL J0654.4+5042GB6 J0654+5042?ïýAPF-P?,@ p=[c?5õ}]U–7?,@ p=[c?ïóAŸBâ?]'eïÖÄ?Y|Àó‹4Ÿ?]'eïÖÄ?ïã"Îzæ•?lœRSp3?lÝ1º³RÒ?lœRSp3?ïþ €#âï?hÙß?%øaÍëk?hÙß?ïþŠY,8?"ù¼¨§?'ZkôÏ|K?"ù¼¨§?ïÁ¶ÜJ™+?"¨±Ô<Çu?$'ºg}?"¨±Ô<Çu?ïÇÜb
ˆ¡?ƒmohDlT?|ϸL?ƒmohDlT?ïüÏOøª?,G¢";`Ú?9…~wÞ›?,G¢";`ÚAGN4FGL J0654.4+4514?"z—ÿCJ5@3cag#$ÈÀ8ë¤dζ²À;ԕ"´@?ƒ*+ù@vÞüz9'?§[ADT?´‹¿f\ÖE@{…L»@'M³çùy¿Üs k°R¿Úd_ó.á¿ä£PÂe?Ë¿ãHÑ?£.¿èåo®¿â	Y€ù»AGNFSRQ3FGL J0654.4+4514B3 0650+453?ïþì¯/?!<	¸7"?.Q2,bœ?!<	¸7"?ïó±=$M½?Y"õÌ	€?X†8•Õ?Y"õÌ	€?ïë°ò?'Õ?[VÄ$å%?dO
¸/ó?[VÄ$å%?ïÿÆ_Üo¾>ñvI½"n>üОãM»>ñvI½"n?ïýõ6ÃG?'͌ါ]?0Sc/¶??'͌ါ]?ïÁÔbåŸÏ?‹å6mRÓ\?Îl3ؾ?‹å6mRÓ\?ïѶƒ+»g?zÍݑhº(?w$¾‹ÎxF?zÍݑhº(?ïÿ—~¦?µØt¥o?
 R»Ô4?µØt¥oAGN4FGL J0654.6-4952¿Ý}ãWu)DÀ3è÷‡‹zÀ:™7ÿJÎZÀ<{OnÓr@JRÃFfA@:6\³_?Àª$@ÒA?š;aµ_?×e …±…@û7Ä<…?ïàÝÆTe¿Ž×GWµý¿é´V~'ÖW¿á	Ò¾@î¿ì˜n÷. &?ÊSØÚ¢"AGNbcuSUMSS J065518-495205?ïîör¸"@?[ŒU͊·|?a	J;o?[ŒU͊·|?ïò‰úŒšû?[»Nw=Ãj?Zì
ä
Z:?[»Nw=Ãj?ï§]}šÆ¦?€%þٚ©¥?†( 'oj?€%þٚ©¥?ïéÞ,5¾?N#ؘo\®?f!ã"™¦?N#ؘo\®?ïa9"(ôô?"rÉ쵯×?"ØÍzáas?"rÉ쵯×?ïÍ%©«?'¶µ9ÚUš?yrm;‡â'?'¶µ9ÚUš?ïi':Q?‹lO÷s›?'ÛZtc×?‹lO÷s›?ïŒx¸Ö¤?w%oðb²?ŒáÑðæõ?w%oðb²AGN4FGL J0654.7+4246¿ä¬Ò@2›ðgȗÀ:VÛó±=$À<XÌ'=«@ P2O2˜.?ÿ†'+½óì?¾K'Ð|°?±ôŸÏ"§?õÓ±Þ3ý^@Y?E:G?á5av<??ã+žI+Âü¿å(M[Óem¿Úà
Fe¿ä¡C§½¿ØÉB>=þ=AGNbllB3 0651+428?ïþt24Ž0?!0	?<SŠ?(¼Ú?þa›?!0	?<SŠ?ïðq¤s?_zOVžU?_·:Ó1^?_zOVžU?ïø+S|+?Tg¯²¤ÉI?OR²"´R?Tg¯²¤ÉI?ïâ:`Ï;?Q¡O:ˆ?mÅ 
/"?Q¡O:ˆ?ïþBž"²?%
æxÝ?+ÖB—b[?%
æxÝ?ïÀJ«…?ƒXö¼Œo.?Ú÷›Ï<?ƒXö¼Œo.?ïû²€›Eì?M ¯s1?A5ýóªÑ?M ¯s1?ï˜#(_Uâ?t=O©øì?‰÷5õè÷f?t=O©øìAGN4FGL J0655.4-2631?³ãç<6ÜÀ%Ý)V:Ÿ8À:u	A}À<8$â7˜@JÎãþAº@KCË0ë?ÆHÆÃHi¦?ÉÙ¨¨UI@᤽º
R@(…a8ª¿ìS^¡Ëí)?ï÷Ìàméh¿â"¤¢Œ1|¿åF–Qæ|¡¿æìãË¿ÈÈf¶˜WûAGNbcuNVSS J065523-263041?ïâ´^ۜb?•n	›?mK¡¦mè?•n	›?ïä£Mw'?níÇzœ¹?k\²"^`i?níÇzœ¹?ïÒì:ó"X?vóT "(L?v‰â–ˆ)?vóT "(L?ïÈ_;"˜½?^zì¾õ?{ÐbN@å)?^zì¾õ?ï¤[p'ã¹?"À³žYp)?†é#æ&I?"À³žYp)?ïb
ÉÓ?¦ÿB?–h?"¬]#n/Ž?¦ÿB?–h?Ÿ9?›÷…`'5(?¦?¤T ¦?›÷…`'5(?îb"ª$e?•d<§•ò?©ÝÕ\+­?•d<§•òAGN4FGL J0656.3-0322¿î´¶ ôþU¿Ý
ÍÞo·sÀ8S&ùz«À;‰ó3hã@ð¶ÛS@WwJº8v?­\ãã?ΔBWC@´'¾‹Áj@°'¹%{¿Å)̗Àñ¿á
Hï]¿çåàϹW¿é¤''¿ëÆ?wå¿ïÿù_|è3AGNfsrq3FGL J0656.2-0323TXS 0653-033?ïQ¨Â!?¥z;Oš,?•Êþúâ?¥z;Oš,?ìpíXï—?Àv—@½¤?¼`•8ƒL?Àv—@½¤?ê6Þ¨0O?®JÿO"tl?Ç$…_>ä?®JÿO"tl?e~#?ŒþÒû²_Û?¤å{_ëÐ?ŒþÒû²_Û?ëùñÀn'û?Á©tó‹Â?À8þE¸?Á©tó‹Â?ÙMî½ÀQ?Òg֐<p?ãYý!Ø?Òg֐<p?獬Sì¢?³¾Ïƒ^¬?ÐåÀ§X&»?³¾Ïƒ^¬?àÀ´´A!?¹Äù":âª?Þ~—þ—}¾?¹Äù":âªMIXED4FGL J0656.3+4235¿Ø_‹¼óL@2Ó~=ÁÀ:³pޏmÀ<P%üu@ Ë­R3(¡?ÿyó$÷0?Æ>oçÄtå?º¬³æ?÷5'm,S@œèwx1•?ïù-Œ*E¿åùy¾‡å'¿Ñâ<xm¿áÄcq¿`¿æ"À%?nçcsdH AGNbll3FGL J0656.4+42324C +42.22?ïý"¨™?(ál)xÖ?3"Y4'?(ál)xÖ?ïì'EÎ|‹?dO6¯‰?cmº5¢ü}?dO6¯‰?ï÷m§Î:¶?T@wƒ‹
™?Q$°4Ïä.?T@wƒ‹
™?ïÓÛÙôÂ?V]
<Üä¤?vx#ƒ¾Â?V]
<Üä¤?ïýH՘?2A½ú?7wËý[½?2A½ú?ïµa£U|?†'è	:Ҕ?'§—BGè?†'è	:Ҕ?ïøþUIÍB?[Ù[¯µÜ?L«E¤ür?[Ù[¯µÜ?ï3³6ßÌ??pF|½?™‰™or)?pF|½AGN4FGL J0656.3-2404¿ëËÇû#DÀ#d¶0©À;("VÀ<dYV³jü@ €õQ%aŽ@ŸKÚÉå'?ÆrÜV¿H¿ƒ¢õ
ÐY?Àh[3,}@aþÍ¥æ¿æCé>GŽ_¿äڔk\om¿èI.p•¿£ÛÔQ¦eÛ¿ëlé7fž›?ÁÂkŠg¢|AGNbllPMN J0656-2403?ïùGÄ\2R?Aù¹¡$8?Jàï'&ý?Aù¹¡$8?ïó—½Tƒ?V"«
Æ?XЅLÞ:•?V"«
Æ?ïÒ'ÞAó?u[*‰4?vþ·.ž?u[*‰4?ïù*ë³d=?5èç¼Bgî?KTQ£"9Õ?5èç¼Bgî?ï÷±fX¾L?N~:òxO?P3Òtgj?N~:òxO?ïЎԪÍÛ?€Â
‹Qñ?w¸•œ*¶Â?€Â
‹Qñ?ïçr,Ã,?tÄVâ´ól?hÓsÍ/³?tÄVâ´ól?ïÐtw©¸S?nžˆS¢¿?wÅÄ>a¦??nžˆS¢¿AGN4FGL J0658.1-5840?ÊÂñRyZÆÀ6 ÝDÀ:Ó"d®ÖÀ<šU¦$ÂW@Rmⱑ@S»¹/?Ã,hÿ?´ÂÖÿ«œQ?ðΩ+Ç?üäò7ëSÌ?捻å'6¦¿Ñݦ䱿ÛY—á]¨}¿ç¼o¢OJÁ¿æ¢nŠ!V'¿Äpêù³Š±AGNbcu3FGL J0658.3-5832PMN J0658-5840?ïü	ÒÖjõ?5ÈùLÛ´å??±gq«'6?5ÈùLÛ´å?ïå"Ÿa…?k¦"0±ï–?j={'Û?k¦"0±ï–?ïà\°žÝ•?o=Á\ÑD/?o£O$©KI?o=Á\ÑD/?ャ«ÅH?a.'!C´B?€"ÕyÓ?a.'!C´B?ïöÖÜGª?G»Ï±ü?RRGüëö?G»Ï±ü?ï£~gdN?'H
'Œ'?‡ f1J@d?'H
'Œ'?ïÂ^¢€P¦?"ØlÄ ˜?~Ю§}.?"ØlÄ ˜?î'üý?Ž3"ÿlaq?§öà>(?Ž3"ÿlaqAGN4FGL J0658.2+2709?ë_ߣí@*ÍA·ZtÁÀ;½x›óÀ<…®
iæ@M†›@ì†;?ȌÇÀ'?yuD½®¨ž?ªLõbSmw@ÄØÆU9m?ïe€Âø¹¿×Ñ}
§¿æ̝Òä>¿ÔÊ#$G]¿é"Ì«>Þ¿Ü#"$ÓAGNbcuB2 0655+27A?ïúÎV©sÆ?BÔȖ:Ö?DƤ±÷;à?BÔȖ:Ö?ïò§AoX?^´¹¥éŒ3?[ü±ëÎ~?^´¹¥éŒ3?ï嶸/Ô%?rI¼Õ½p?jIGÔKb|?rI¼Õ½p?ïù¦Füá?+€q̈́â ?Ifãªhê?+€q̈́â ?ïõݦ¨›?PhÕ(&ië?TD²j(›]?PhÕ(&ië?ïµ»¤±?‰eFY?\B?'¹'Ã%´?‰eFY?\B?ïÆ5ôIz?"ˆû¡'€Ã?|åt–Yc?"ˆû¡'€Ã?ïé4ðw¢?RðÓ?F¢?fêËÈ®7?RðÓ?F¢AGN4FGL J0658.6+0636?ëó'õCA&@j¶ÂŸLaÀ:R"ÅõB7À<+°¶ì'@ °jûw?ÿKXÃæt?Ã"ÝûsS_?¡¬ØwHP?ßmõܐ/@Ûäkyö'?ä'6ÎÉ&O¿ëów'1L¿Òˆ:̄¨¿Ú#ìnRÄ¿à¬![š[¿âžf½¤:ÝAGNbcu3FGL J0658.6+0636NVSS J065844+063711?ïúEpD0?<1qg u–?Fê?9V·?<1qg u–?ïè~Pýã?sc'ËgÃ?gåyh5?sc'ËgÃ?ïó˜ÒZ''?Rõö*£?XÎ[Ö»U?Rõö*£?ïéɓ˜‰à?J#¢Ùøœ?f6lMYÕ?J#¢Ùøœ?ïöâÈÀ+\?G¯ÿ"?R:nd,gw?G¯ÿ"?ï¯-ÌäA?©(«è-?
IÓÖ?©(«è-?ïðšçé^?nœžg!âÕ?^ËØ^çô?nœžg!âÕ?ï´oR•›€?l[C_?'ä+XáR?l[C_AGN4FGL J0659.6-2742?ïÿ¿[}²¼À%/UÞXæKÀ:3Æ&À^*À<3"'ʘ@X‹®õKq@ÚíÜçÍ?Â\ÉŃ"?Ӑ{xFb»@íÅÖ8†Y@‡¹Wzf?ïû7mª¿Ü´>¥¿ç(Ãm¨z¿èjÃQ#¿éÿcøÍܗ¿ðAGNfsrqTXS 0657-276?ï\…@évž?'ãšC¸'?"oWßaC?'ãšC¸'?ïÜhu#1w?oÖ÷&^W?qËÅP*´?oÖ÷&^W?îEÍDy?›~tЛ•?«£+¿{Ÿk?›~tЛ•?ïªæúå'Ñ?c°dÿa‰-?…FACFo´?c°dÿa‰-?î™'Ù¸Ä?§U6?ç}{?¨m…ÔÃ?§U6?ç}{?ïGY|._ö?‹tåEš?—ÐvÄeG?‹tåEš?ç¶|£?´¬75^L?ГÛçĺ?´¬75^L?íA͎Nóê?˜3ÚauŒ?µñ"ŽÒ;-?˜3ÚauŒAGN4FGL J0659.6-6742¿Õú
å#ŽÀ80…†"À;Z©Jç"ßÀ<¿<ÓÅåR@"0ü@ظ=?úƨZý|˜?Æuøˆ‡?œãg‡½gï?×p§\û®@á*ŽÉÝ¿ÌÁ¬­O"¿ïúeA"_%?ïú¹¤ÑÜ¿âït'ƒ¿Ü»©ú9íb¿›…
›tAGNbcu1RXS J065933.5-674356?ïþºßJ¹ô?
$Â؟³?$R#A0b?
$Â؟³?ïößá/8?S"–ÞÄh?R@=¬Ž¶ã?S"–ÞÄh?ïðiÉꑦ?gû·\ZÈ?_,lwÓóF?gû·\ZÈ?ïú!8	?8"Qð?Gÿz''_ž?8"Qð?ïýþ«õšT?(árÆ·"¨?0
¢8Ö¾?(árÆ·"¨?ïÕy¢¿nQ?"¶tÛDõ?uC.—YÛ¹?"¶tÛDõ?ïöÉ0=¾?dÐMüˆ_^?RmŸ+?dÐMüˆ_^?ïó‰óðcf?RLÏHHŠ?XìV2ó?RLÏHHŠAGN4FGL J0659.9+1709¿ëS;Þe@#¥ß"9çÀ:4\|ؙÀ<‰£–@(ÄBd©x@#«äøê?Áï,ž¯N?¢_ä°Þ?ÝÛB›Ûé@
=‰T'¨¿áë5@L ¿æDI,«¿æêò®~¿çbår¶¿ë	3ðÈT˜¿ïÿHë+\¥AGNfsrq3FGL J0700.0+1709TXS 0657+172?ïü&n¤4?0I];zl?>˓9Qä?0I];zl?ïï
¨Ej)?iUœxmc?`òWíp?iUœxmc?ïæµoý­¯?g"QÊ?þ?iJõó¸ý?g"QÊ?þ?ïýf<ldO? ©sQìfÝ?4Ά€³ð? ©sQìfÝ?ïûÉoJ:·?7Ÿùb6	?@ÚAñHà?7Ÿùb6	?ï áŽÃE?'RÉL·?‡Çœ{.¶?'RÉL·?ïæÆ}IÏ#?nGãüa¸s?i9'Ó
"w?nGãüa¸s?ïö¸†ÍB?EŽ(ö/F3?Sҏá@?EŽ(ö/F3AGN4FGL J0700.1-6311¿îÀ½Þ%oÀ7·ª%ÙÀ:±ñNŒU
À<˜M×ú'y@ )ƒ:1ª?ý'-ê
Ë?Ƃ_UÐìí?ã©'#V?ýÖ—Péý@ô
8"x¿ì(ǀ?ïúªùš‹¿Û["ÀĀοÚkaýËó¿äãacÈ&¿ìó)WèbAGNbcu3FGL J0700.3-6310SUMSS J065958-631238?ï×®¤\…?¯´ö׸8@?t(­´0Ü/?¯´ö׸8@?ïóíðU_z?X±ærµ\?X$ZÀkB?X±ærµ\?ïîXÑ['?gVô	Òé©?a§.×Õ¦§?gVô	Òé©?ïðÔG%¿"?A€$µ%Þ?^Wqg‰™¢?A€$µ%Þ?ïüœ@=ò?4ž'\=r9?;ýè?4ž'\=r9?ï×õD'Ö?wLh"gõ?t]ÉÊù?wLh"gõ?ïé‰Õðüœ?n…C¸ôÎ(?fv)ûŔd?n…C¸ôÎ(?ïÌ£ÌoÒ?jz·µ:0?y®ؕ;?jz·µ:0AGN4FGL J0700.2+1304?Ùhš%äÕ@h>]2àþÀ9æGÁ_±À<(É Èb@Þcðë: ?þ«rßñm?ÀéðÊ1?¹ù]ú\'?û±ƒ›*"?ñºØ®'_?ëKg<O;§¿åj(3¦¿àà Ç`¿ÕZ¤k¿äÐeÁ•a¿Öi}±ÇAGNbll3FGL J0700.2+1304GB6 J0700+1304?ï÷@ðl©?Pc*d]Í?Q~³)-»?Pc*d]Í?îÀgSÌr?£Õ?JäAî?£ùŠÑòÔÞ?£Õ?JäAî?ïÕ- f?ww
­ÀÞ{?uioÿC ú?ww
­ÀÞ{?ítXق_?"{©°M<?´_E9¡à†?"{©°M<?ïߓÖáù…?kßÿZ]?p6¤Pх?kßÿZ]?å@Œ!-n›?Ï®Ô7éë?Õ~ç½¥"Ë?Ï®Ô7éë?¿Nµ?‹BV͑û?‰»QáZ^¬?‹BV͑û?ä|Ecü?°½ðx{üK?×ÿu8?°½ðx{üKAGN4FGL J0700.5-6610?îzƽMÀ7–6—lÀ7àóÌëÖ}À;n,Ñð"@zrè)õr?ÿlV…GÒý?˜´C÷ä?³èù~0²z@H	N][%@J	99²~?¢‹>šÖ—¿Ø}å,õ,¿àŠò×ùP¹¿áQ¦ é4¿åó`	€¿å™
Æ(ÄAGNbll3FGL J0700.6-6610PKS 0700-661?ïüOR½Uû?:dU¸[?=…kݜDn?:dU¸[?ïëÏÖ[Z³?v}£ƒx&?d0)pk<Ú?v}£ƒx&?ïØ@èlTV?|ôÁŠ…ɾ?sߋá3,ñ?|ôÁŠ…ɾ?ï÷ú!³s?@"œ1Ñj¶?QØ@Š®?@"œ1Ñj¶?ïû¿oé??9µÞÁœ?C­Ûù??9µÞÁœ?︑'Ëý?šH!ÄÛC?Û›{¬ØÀ?šH!ÄÛC?ïÎñS®—œ?"`ؗ
:?x‡VC%¯?"`ؗ
:?ïÝ:@¡8}?aèu§Nq~?qbߜÕݛ?aèu§Nq~AGN4FGL J0701.5+2511¿ì¨Jžoþ@*ˆšgó
À:ñ/¨;ôÀ<‹5RÈ$@!""«þÎ?ýïüÍE˜'?Â`#×·¿"€-Hâ$?ӋªãÃß=?ÿ8·§ ÀÀ?ç–_½Õ¹¿ë%d`ãð¿šÚ}xg¿éCN¾ÿږ?µÝ´¦M¿Û'@dtßAGNbcu1RXS J070132.1+250950?ïþ(o¾\z?#ÍRÃ/§=?-y+Ïöa?#ÍRÃ/§=?ïîÏë݀œ?b§~ÜÄY"?a0_Ür?b§~ÜÄY"?ïëïÙ°ú£?V³ß÷ê
_?d&?ç?V³ß÷ê
_?ïùL®É?4äÒNfÝò?JÍDó9¸j?4äÒNfÝò?ïûs2Ÿ
?9QzZ÷j?B36%ˆ O?9QzZ÷j?ﶀì‡?Š³½|å¾<?'|Í.(S?Š³½|å¾<?ïåU¾½.c?sÃù¸<ñ?jªAƒjD£?sÃù¸<ñ?ïãßM'ê¬?a­oöÆ8?l ²'"´s?a­oöÆ8AGN4FGL J0701.5-4634?æGsJê#À1´ÖÂïÔ9À8ýë7ñÞÕÀ;íhò1á$@àht³†@‰bI¡3Â?©¾X»æ?Äâçxb<@4aQJ@½©›ð6¿Ì~UE¿]¿áŒ†'ø¿å‡)õœÏ¯¿ç7?#Vq¿ìíÝ|艿ãšÑ½woMAGNfsrq3FGL J0701.4-4634PKS 0700-465?ïç>×<x'?fÙ1ØÜ!?hÁ)í0?fÙ1ØÜ!?ïÞñ_?nªÄøé?`j#ÎQ?nªÄøé?ï;IQOo?"JëiMª?˜–ÕÏ<Ú?"JëiMª?ïýW浛?%_¨šV?7¥@÷g¡Õ?%_¨šV?ïÈEç?ê§?v÷m?¤§?{Ý|7x…?v÷m?¤§?ï»*úeÈm?•qsÌÄÄ?5AW¦Ö?•qsÌÄÄ?îNÔìÖØi? çöP­+B?«±5&.f? çöP­+B?ïñPJl?Oii‡ò'?]_óš"×õ?Oii‡ò'AGN4FGL J0702.7-1951?ë4¯ÜÉfˆÀ_9K{)À8°µ "µÀ;q׉¿1@êwY¨½Ï@ ºK?©ôr-Dé?¶Í´~La-@
ۇz³%@b
Ë5¿ÐìK¢ë§Ù¿àÏ9#7<­¿ÞÕPߖ~¿àèuÕo2¾¿å,‡m¹—¿æ¢Òþ?5 AGNbll3FGL J0702.7-1952TXS 0700-197?ïþ-Hý8¿? ûLO3Uµ?-+nS©Ð? ûLO3Uµ?ïð?J£?k¾‹·e&?_Á¼j4?k¾‹·e&?ïç¯Ápš"?n~/#i¶?hP>uHcì?n~/#i¶?ïýÛ»'2õ?PgñòUï?1"(¸|ƒÊ?PgñòUï?ïþ)özü?#oÛ^ì&?-`ž¿]úb?#oÛ^ì&?ï€Ï§âK~? «&!oH?Ìù®°—? «&!oH?ïÞÇmMG?|%Μèœ?pœI‹ˆ¡?|%Μèœ?ïú`;݄^?9LJ¤ê"o?F-ý1?9LJ¤ê"oAGN4FGL J0703.2+6809¿î×®pHðè@:.Y¯ž¿À;Äp/=mÀ=y@]¾!@!m›
à?þÁX$"D?Í¿9?«BNâ™ÆC?ß:#<p@#_•'Í¿é(Qû,Ý¿ìÎÛÐuι¿¦èsFs­¿Ý»ˆÂ0ç~¿èóá
Ìq?Øߓ£áF,AGNbcuGB6 J0703+6808?ïÿ3 ‹2E?4Ï­÷?›ì4"?4Ï­÷?ïô¸Ê?"?WÎx"Q?VŽkç§h?WÎx"Q?ïò£"¯W?nL"Ãi»Ì?[øº#p?nL"Ãi»Ì?ïüÉ)\Î?)ßraÏʽ??µ\óã?)ßraÏʽ?ïÿ|áÁÀC?)PÓÆc?cÐ¿=]?)PÓÆc?ï×òýÛ?tjþ¿£Ås?tsu#]Ê+?tjþ¿£Ås?ïíSr^d?tèÕB?b¬Žüs?tèÕB?ïðŠ'û`x?Q©é8Œe3?^ë°itÓ?Q©é8Œe3AGN4FGL J0703.2-3914?»L*%'—À-J×ùP¹VÀ9Àø£lŸÀ<6¦CÌ«@b'vŠv@|_ag?´ÂüÿÅr?°uŽbÿd?ûBJÈ{.u@Q&úë™?ïñöó4¿ãå"~°	H¿â´½ý&¿×ÇÚñR¾¿ç$¢¬gÒw¿ß	žs`AGNbll3FGL J0703.4-39141RXS J070312.7-391417?ïùÈ=›ìÛ?=æF›ÿ?Hß
ƒ×Hì?=æF›ÿ?ïî™Ä?h(?^jÏ?
‡c?af;Òuρ?^jÏ?
‡c?ïì¿£eí'?e ™yùj?c@\³Ö?e ™yùj?ï¾^ê
;?dãåÅ͛?€hEl¦[q?dãåÅ͛?ïè‹»?c"'^¹¦¯?gîtg[?c"'^¹¦¯?ïÉh~;Å?}Ø2Q¦Ö?{KÀÀ…å?}Ø2Q¦Ö?ïËJ‹`é?'""¦1?zZº^©º>?'""¦1?îø*4B8?ˆM÷‹? }\»Ü~_?ˆM÷‹AGN4FGL J0703.3-1042¿ç=¡>\9ÅÀ'D`'!À9j‰r¡À;HlÞO¬@¶6]_,@5£]gº#?»€;"n?"‰y­ò?ÙSËäÅfý?õ˲BÝË"?ïìfZ§ìC¿»ª¾–9y¿ë0Ď9ê¿é;(àsó˜¿Þo+|/¦a¿Ô‡B^Ê:ÌAGNbcu3FGL J0704.1-1043NVSS J070322-104426?ïõ†ûî^©?\øHF#?Tò‹¶ÍG?\øHF#?ï¤þçsŽ?ŽvÀçìVä?†ÀF͈2?ŽvÀçìVä?ï"lÐ҄¶?&sEí¬?›²eçg7/?&sEí¬?ï]µA¸(?zuˆ"ps?"IW´`?zuˆ"ps?ïdØ,ì?'°1çù?"|äýÒ˜?'°1çù?츷›Q?ÀýÆ굕ù?º:C%w;~?ÀýÆ굕ù?íÑÖmE¹Ú? ¾ý)¬ŽÎ?±qL"c5? ¾ý)¬ŽÎ?êW÷´h84?°Ùüzê?Æ !._1?°ÙüzêAGN4FGL J0703.3-0050?Ä8'©Ì~@ø/0oÀ9ˆ²1@ìÀ;—'?2D÷@dn9ïdý@ƒ¯à,ûâ?¹nÓâ¯|?É'ÄÀ
÷@~…vÌå÷@
Àöäxe¿ÝO©@U°Œ¿ÝÖ
RÎÙí¿áú4CÔk'¿ä>¥¢fqÏ¿è1áÏh^¿ï÷:Êi²AGNbcuTXS 0700-007?ïœý–?‰_sâöu?ˆÀšTùƒC?‰_sâöu?ïÀY¾Ú"+?ˆÓY© •?Ó wévt?ˆÓY© •?ïvÖÑ]€9?ˆ¾{F	‰?'%%Ùwbà?ˆ¾{F	‰?ïÑ/N†?W=n0ÆW¤?whYÙ\?W=n0ÆW¤?îÆ
,öûl?£SH¤~x?£Ÿ]2H??£SH¤~x?퉻Ñ/š?»SQ¶«ù?³²!v‡±?»SQ¶«ù?êæÉø~xÎ?¯¦Ðã؎?ÄdØÇ?¯¦Ðã؎?îvMa‡¯a?'$G¯'iE?¨›)ã9†ñ?'$G¯'iEAGN4FGL J0704.7+4508¿å
+Ž¼=@5I˜ˆøÀ:ÇG'u¦À<hÇñ›¹/@ŠÒ¬_Å@@Ÿ}i[?ƲŸzQC?¸fœ«fK?îÑ;ÇVkG?ú"#xÕÿ¦?ÑØ	âx¿ã¼Å¸ÜU¿åX•Wëy`¿ê	âÂW}ë¿Ö"%>(¿ïð4í0EAGNbcuB3 0701+451?ïüăN?2' ØÆÑ2?9Ûç…mՙ?2' ØÆÑ2?ïÚÏÌRö¿?{  ð.1‡?r˜êr\6?{  ð.1‡?ïÜV¼ûì?f/Àª…K?qÔð° R?f/Àª…K?ïʯ2ªn ?_¦â"x?z¨fËŸ?_¦â"x?ïú.4ÏH0??Þ©ë4»?GG-.7??Þ©ë4»?å(?¨C²­øÝ]?ÎɃ[?¨C²­øÝ]?ïµ?AUØ?ƒ"ée¿	†?'°/´ØÍ'?ƒ"ée¿	†?íþå¬JSê?œ'Ä`r?°ҟÓ"/?œ'Ä`rAGN4FGL J0704.8+4907¿ÏtˆŽÀˆØ@6BÅ;ËÀ9äz[ñÀ<8>gCÛø@¦¼õ¿4^@'8å#Û§?µ}€´Elq?Ö=C­Sá@
bô ά¡@.-ú'ѿ͍òÇ]L6¿âu۞÷§l¿ärB¬^¿éÍÃ\Ⴟ彵½¼Ž'¿å°eùRAGNbcu87GB 070112.8+491056?ïôÐÞÍ*?'8Ê\g,ˆ?V_þ!ikX?'8Ê\g,ˆ?ïó°b¢¦L?YÖÄ Âþ?XŸ;(Ɩ?YÖÄ Âþ?ïÌÉJ:?²;ò4"m?yþ›ç†É?²;ò4"m?ïùà֑i?/GOÒºÌ?H|¥O´•Ë?/GOÒºÌ?ïøŸ«xá‹?LJd&sЛ?MR"9!Î?LJd&sЛ?ïÇ&? Š0'fl?|pó{Ãàâ? Š0'fl?ï3Ukþg?"$#
?™œY_k?"$#
?ïßµ:ðýë?ZÅ{£{!	?p%bqƒŠÂ?ZÅ{£{!	AGN4FGL J0705.7-4848¿´õ1ÕAÀ1Øc8´|tÀ9Ö­ò2qÀ;úˆFŠþÌ@âs'?	*@Oï0l¯?¶®|Փ›?Å?Û¢¨‹û@
3Xòà\Í@½^Ä»?â—m¿öûu¿ÔB±Á¯¿ãx†YJôñ¿åûŸíp±¿çŽëUN.¿ïþu]AGNbcu3FGL J0706.1-4849PMN J0705-4847?ï™Lÿ¢¯?"=‹Ä]?‰¬ùÊf(?"=‹Ä]?eçª8?Ï½§d	?[&{ƞ*?Ï½§d	?ïoÄÇÖÔõ?‹ö?Ý.?'füŽ[x?‹ö?Ý.?î÷è"?u`U=é¬l? Á{üHè?u`U=é¬l?ëƒüӔ€ð?¼ö–ʲ@Z?Áð±­üA?¼ö–ʲ@Z?ìä²d@ÇE?·[Eµ'©?¸Úlß±"Ò?·[Eµ'©?éÚ²甓?³ˆÖ˜/ß?ȕ7äa­´?³ˆÖ˜/ß?çŽtÇt•¡?§ùÆ:mf?ÐãqÔ¿?§ùÆ:mfAGN4FGL J0705.9+5309?î¡k➒Ÿ@7€ZpŽÞUÀ:Ø	ٝ•¨À<³Ð¡m£r@ÁÂr«Ä@'6~AN?ÁÂ˗´'?¥ùiãÉh"?åe'
@ž3ƒ:1ª?çÛ-¸Ÿï¿×å°¿åï
¿[J)¿àñ¦&oÖ¿áúw?|—«¿å¡àåÞlAGNbcuGB6 J0706+5309?ïý¤Ñ¹¤/?#§ßbdo?2Ùq·¹XC?#§ßbdo?ïôþäÄ\³?W=`_šÓ?V6Ô»ù'?W=`_šÓ?ïö±ÅŠcF?\5Î(¤‡\?Rœt©@ôÆ?\5Î(¤‡\?ïõ´Œ†ƒ	?3²wO\•?T–æ'F¾ñ?3²wO\•?ïû†ÈþÙ\?5t6=ÞÕ?AäÜ9a]`?5t6=ÞÕ?ï͍ÆûL?|·
lbMV?y9@ÉÆ?|·
lbMV?ïõká}ù?d éŠÂÄ?U(Þ	
?d éŠÂÄ?ïÙÀeÇ?[F'‰e?sw@/›P4?[F'‰eAGN4FGL J0706.1+0246?´%Q|­!L@.beOæÀ:ýž5	ÍÀ<SôH;Øô@#½ÙI\ë=?ù"¡ò?ÄÚUv
Q?†o*bÝ£g?Â`|-Q?ùœÅˆŠÓƒ?ïMú^ÖO-¿ð?ïÿþó…õ?Ôr‡qxé ¿çää†&ö?ˁ%D@çAGNbcuNVSS J070610+024449?ïý»|ÃJ?&Ì5þy?2$O÷¢?&Ì5þy?ïÛ ´.à?wÀ¯	¦È…?r/¥É£ƒ›?wÀ¯	¦È…?ïñ:}²æÐ?X"ðªv…s?]‹€p>?X"ðªv…s?ï£æÇþ9Š?{N´õ¾Ô)?‡NPÕ{?{N´õ¾Ô)?ïýgÝ	?*'¤s€6?4Ág"ðØ?*'¤s€6?ïAºUYY?¥rPzLêm?—ȵO¨jà?¥rPzLêm?ïë!ƒ­¨?p=ïýv?dÞé[V?p=ïýv?ïMùTŒ–ž?ÛK$G†G?–@ÕqÜÈ5?ÛK$G†GAGN4FGL J0706.5+3744¿í#`Ê<œ
@2üð¸,,À9'dö#Þ,À;Ӝô—ìñ@ÍëZ×g?ü=³¥Ýu?«–3Þ~Ðë?°rõjû¡w@ƒZ'ó@=«2ž7ä?ïæ
öÔT¿Ùº"ÛÍпٔPdF{¿Ú&Y›|Ȩ¿Üž^$x…M¿ÞË(~»ÈAGNbll3FGL J0706.5+3744GB6 J0706+3744?ï÷¤ˆS)?D\ºa4]?P¶ïX¦~ì?D\ºa4]?ïÇ2@fnì?|\©oî¯?|fß­,"
?|\©oî¯?ï…ܽcV?Š'JC:ÕN?Ž¸ˆÐ§*"?Š'JC:ÕN?ï0Çóõ?€)"ú)Ç?œ9ç_f?€)"ú)Ç?ïØ¡]Ìþ?i"ŽBg?s¯Q2íÔ?i"ŽBg?î¸ ¨lZ?´7Á÷×t?¤}õ{ÒU?´7Á÷×t?ï}ý(¢?–3ȦÄǽ?Ÿ@TƒåÓ?–3ȦÄǽ?ìxw_cÛ?¢Ԋéúñ?¼<Eá*?¢ԊéúñAGN4FGL J0706.8+7742?»žŸ¹yC@;Gy¢ƒMÀ9kQÄòÀ<,=ÐE'Q@¯"}ûÙU?ýıû.·?­òŸïV?¾kdÒèoÁ@"ïï@Ÿ|󛘢¿ÀµÏš²sZ¿Õ‰æ]Â}é¿ÜÙhrLN¿ÜlÅP+¼¿äô,ø†Žû¿è"3ÿ
zAGNbll3FGL J0707.0+7741NVSS J070651+774137?ïý_ÿÄñ·?0áY¦:½?4ÿÿ¸0*d?0áY¦:½?ïñßxËî«?]µIU¾?\AL¥ÉH?]µIU¾?ïЈ4±&m?xÅ%хJ?w»å'oI©?xÅ%хJ?ïü†ôPtb?$%‹GB?;È\ì"?$%‹GB?ïýò•3X?6–œڇ?78kwa|B?6–œڇ?ïÇóÿ¡?~‹R¸˜e"?|vxï‹W?~‹R¸˜e"?ïɒ­cV?†ú½™`á?{6©7ƒéF?†ú½™`á?ï÷n.÷¼?=øé-å¬Ù?Q#¤mÇæ?=øé-å¬ÙAGN4FGL J0706.9+6109¿ØâµÜ	E@9^=áâßÀ:>pɖ·gÀ<'UÓø@¬¿y4t@,ÅZèƒâ?µ¢7¢Ù‰I?ËPÿT'?Ö<á>iÈ@"IX¹"?ï &Ö@¿äȒ@	‹¿ç>-—è¿r¿áÒ6™A¿ç}§á¿åmü\ÝQAGNbll3FGL J0707.2+6101TXS 0702+612?ïþ:~½0‰?…¸Óå2?,XùuZ?…¸Óå2?ïõ»QÄ?TqÜþ&˜¼?T‰^g,G¦?TqÜþ&˜¼?ï÷ú Îå?:OŠÞyø?P
¾³y%›?:OŠÞyø?ïñ'Ø›sJ?E"Jî_³?\ÚNú"ÌR?E"Jî_³?ïý05ˆ?1'cՉ¢_?6|Ĩ&?1'cՉ¢_?ïÓK0wc†?x†mÑ?|[?vZgÜ[€Ç?x†mÑ?|[?ïôÒÂQ–?Z=sqEvZ?VZ{_"±?Z=sqEvZ?ïÒg
G£û?c…XáòÉ?vÌzÊÿö£?c…XáòÉAGN4FGL J0708.9+4839?ÛçUnòQ@6Ɉ;£D=À;IÐ&ô`À<Á½"¨™@!¾¢ªdm?ù~{?ÑΝœ…?Ãfmé~3?õslg@8Ë0šÂ¿ÛšÚŒ¿ïÏäM?êÏlº=~¿ÙèêÅ[>j¿ÒÝWžøS8¿ÞP?þªJAGNrdgNGC 2329?ïþ,+_²Ì?"b–Y(ï¶?-=N³p?"b–Y(ï¶?ïò_dOÆù?\­TüÏ{€?[A6ú½žÐ?\­TüÏ{€?ïñ-ƒŠ¨T?L/¯@i ?]¤øt|Èã?L/¯@i ?ïñ1_ëÅX?F) 6½"‹?]@ˆª_Å?F) 6½"‹?ïý+œQÒ?0ØVyý?6§|¥÷ÿÙ?0ØVyý?ïκ`—"$?zWìYÎø?x¢ÏЛº	?zWìYÎø?ïí•t›ÞB?gwî7!r ?bj‹:æmÎ?gwî7!r ?ïÚ,r`?fßÝö•É?réÆñ¬+H?fßÝö•ÉAGN4FGL J0709.0+4304¿±Äž¤3Ð@5-j½ãû½À;—ߨq£±À<žÌN!Ì@ N33²à@tÛ>—?̳Ä=19¿…˜ô`Ãô?·B›îœo@´h"ÿ‰¿Ø>\œŽ­¿î{ ŠN£¿°©»¿xS¿èä§՟Ú?¦RCí²1¿ïÿ¡ ÏAGNbcuGB6 J0708+4306?ïý¶ß¥—?.–J§›K?2I‹œ@?.–J§›K?ïõÔo¥Ì¥?Vsó[ó–ô?TW @óÖH?Vsó[ó–ô?ïì×ÎLm†?`E"<è?c(1ð™þ?`E"<è?ïþò…)[T?
:¸}Ü? ×±hÖuÈ?
:¸}Ü?ïýœÞr'˜?/h±Hõ¿?3taì?/h±Hõ¿?ïÍ7-Þ?€ò5»CzŽ?ydsfõ?€ò5»CzŽ?ïæ—Ý	Ž}?sZÖÕÐ?ih#%,3?sZÖÕÐ?ïùÍÍ3‹?DRl$x7_?HËÄ<ÎÐÚ?DRl$x7_AGN4FGL J0709.1+2241?ëÒê'äv@+ªºà;>šÀ9Hôá¾ÌYÀ<*2	@Êi©;ù?ÿí…tH§9?¯ΠÑ5+?±k
?-½S@t–'äZ@D!ÂóZ¿äÒ-^ÝÛé¿Üeށ*7¿Ýk¶Eê¿áK—þŽæ¸¿å_(뱔¿ÙQQAGNbll3FGL J0708.9+2239GB6 J0708+2241?ïþ»ò´èÕ?ïúÓP.?$@×ß$Ö?ïúÓP.?ïó—›"í?[ ¡DŽ?YúÐɺ&`?[ ¡DŽ?ïïD¥ÆT?p°ad"".?`»[öÛë?p°ad"".?ïýþÜЌ0? zT(3©û?0	—Õ€ò? zT(3©û?ïþÖ1%Î?"ª…ð²?"ž«µ`;:?"ª…ð²?ï±GË.ù?ˆé»?É?ƒ®
?;Ó¸?ˆé»?É?ïôÛáµ­?e'RÛ§Ö?VH=`DÆ?e'RÛ§Ö?ïü8q­å?1O7ãñðÏ??=eŽÓ;?1O7ãñðÏAGN4FGL J0709.2-1527¿é˜§7«¬°À	0$öYŽÀ:–æ`ò‰À;øªLb@!€¼&'?ûÖNUÎh®?Á˜kܜùu?½j§=Ç
ì?þì¡c'v@Y1(¥¿ïÿÝ/ñ_S?ïÿþBe«+¿ÃGahz½¶¿ÇeöÔÞ¿åK
P»Ú¿¬:XŸ¯AGNbcuPKS 0706-15?ïþjŠbM?PË2/]~Ì?)^Œù…Â?PË2/]~Ì?ï泚:˜?s¿û¼zk?iLe½(ÔÝ?s¿û¼zk?ïßi_?*¸?w¸F]#?pKPO<—û?w¸F]#?ïå6òIM?TÙz{#0?jçÉ ô'û?TÙz{#0?ïþ,šÑ?%2;ë•!?-6Tš–!î?%2;ë•!?ïO	'àšŠ?¢Ð)Ԉڏ?–Ï }Ä?¢Ð)Ԉڏ?ïÃ}Œ³?'‰l
Ï@·?~zAMžâ?'‰l
Ï@·?ï¤Ý—á;?wø'cúO?†ÈœŒIA@?wø'cúOAGN4FGL J0709.3+0540¿ê'…4@@W_bf'À:7a=1¹¶À<1REG1î@KÓòZûÏ?ÿ»°åæyF?Ä@jS…ä?¸HQÓ\?õ:ðFN˜ê@'P(as
¿ïþ`ù?Ÿ?ïîLC¥q>¿çØ#­"2)¿Ð®#¿LÜ¿ãˆ$A'è|¿à8L­W¼AGNbcuNVSS J070916+053901?ïþ·t1;s?c6T?$ˆÀßÕÒS?c6T?ï竚oyØ?sA@µÒ]N?hTeÆ á?sA@µÒ]N?ïöÀN—Æ8?Tá†Å7÷M?Rbàñ¯?Tá†Å7÷M?ïõ°¢¹l·?9	XÇÙg?Tžº	5'½?9	XÇÙg?ïþ±2´Õ'?;:ٙq?$ìÓ·÷š¥?;:ٙq?ï,§õ
Cò?¦'u\E?škZçåÔ?¦'u\E?ïówë±?h{ëhèN?Yú-ùýx?h{ëhèN?ïՊº>æ×?e`‰)§Ì?u:¢ì;@‹?e`‰)§ÌAGN4FGL J0709.7-0255¿ä¿ÞíCÉ@åc>"¹†À8†à66òÀ;q¡3ÁÎl@of×¥mã@¾::ŽqG?¥­ {\?±¹_°ƒ…@	•õB6Ü5@T84ÏÀr¿µVz\'}¿ß| $"I+¿åŽ¨orŒ¿âh‰¡~ëC¿çä¢ Ñ±¹¿ãHhÌAGNfsrq3FGL J0709.7-0256PMN J0709-0255?ïý"¸êu]?,ÉÃì	‰ ?3Ú7ÅoZ‰?,ÉÃì	‰ ?ïá\6PŽ?{‹hjQ?næ£éKÚ?{‹hjQ?ïæìcž"‡?q¥öíÝ?iœalxñ?q¥öíÝ?ïþ=gêtþ?îzÞ¨!?,) ??îzÞ¨!?ïýBÐ#[?.J»_¿1í?5é|çeÒv?.J»_¿1í?î©FáÌõM?±¥›<dm?¥k'ä'1?±¥›<dm?ïÓ?,)˜?{ô«Â÷Åú?vwàe¿Ï?{ô«Â÷Åú?ïû§»Æ???1ëe¥¬´?AaýƒÍ?1ëe¥¬´AGN4FGL J0710.4+5908?îI±Û‰.@9lÀz®òÇÀ9ºÑ4:š0À<6ÙCӔg@!‰Á	u?ùâTÊ\°?°å%´¢"?¯9±$P@º?Ú
¢ñ@
'Å—j¿êŠˆ_	¥Æ¿´#7èy¦Š¿Ô$«°óRs¿Ðpeƒ<Šö¿Ü¡ººÑw¬¿Í_9÷GŸ§AGNbll3FGL J0710.3+59081H 0658+595?ïÿ&IH{ø?f¹æ ?6ؾLsM?f¹æ ?ïôsóþÑ?WÖ8o«ß?WIÕ»y?WÖ8o«ß?ïö"F搻?U"ÿRôU:?RÙr¡úõ?U"ÿRôU:?ïöš…@µì?:£h¶eʗ?RÊõéÇöw?:£h¶eʗ?ïþ´žá4Á?´qÐ_É?$¶qŽ·Â?´qÐ_É?ïË@w¶½8?}$jÒ3¤?z_Ä'ßé?}$jÒ3¤?ï÷™´éÏ?býaÞK??QøÌ*ø"…?býaÞK??ïèÑâ؟5?VPw†[8µ?g.b
³?VPw†[8µAGN4FGL J0710.8-3851?ÕÐ:k.ÅÀ*E{cM­2À9œFp&ىÀ;æ~AN~é@õ£	ÚÊ@ž¥·µ?·ûRò[²?ÆRüýA@"ô%×*@²§|0R-¿á•ú=H_ë¿àƛÞÚ¿çöó<¿ê;3¢™Èi¿çʃÁd¿Êëï½<¶ëAGNfsrqAT20G J071043-385037?ïüó{ë¼Z?3µ"æ?8d",Ö¶>?3µ"æ?ïô™¨ï3:?[žÿú?VÌ­°æ[ü?[žÿú?ïÓҊr#?pÀp:S!¶?v»e6V?pÀp:S!¶?ïü滾æ
?%PB¦V`?8Ê!á:3?%PB¦V`?ïý"×ôÚ?5ë²°CtD?7ƒbè…3?5ë²°CtD?ïÓpy¿?~Î@ç½C?v@Gçtì°?~Î@ç½C?ï[)}õ?•PŽÿ/ø ?žôœ_÷«V?•PŽÿ/ø ?ïèlaÁÕ½?[Å6+éCw?g"ž-¬#s?[Å6+éCwAGN4FGL J0710.9+4733?ï½ÿ$Á^@6Ìt§qÉqÀ9ýçÆ²À<Owï$æi@¸Ä(äOË@ë꺝 ?»ËA1xö?Ãv.^b@*6âëC@y	³ˆB?ï!#}´¿æY*Fy¿è¿ÔáïÛ¿çq·20Ô´¿ð?ïÿÙi"A'AGNbll3FGL J0710.5+4732S4 0707+47?ïù
'ð5?NÞQcºŒN?KËÍ֏Y‡?NÞQcºŒN?ïòñowÞ?[Y ®ÙkE?Z!âDr?[Y ®ÙkE?ïÆ(ÈÂ?wyCÅs²?|ë¹f.ƒY?wyCÅs²?ïöõ³S‡š?=Õ=Ù?R™7\?=Õ=Ù?ïóhÖÈ­?a8®þËÅ?Y.ĎçÆB?a8®þËÅ?ïÇÒÈËq"?€áÄò^þ?|›¨¥Ù?€áÄò^þ?ïE·äÕ¤"?'úļ8ÿ?—Ig=y?'úļ8ÿ?ïÛpçÒ??l~—¦9?~2GqùØw?l~—¦9AGN4FGL J0712.4+5724¿äR±íg:æ@9ZakTãÀ;s\,PÀãÀ<µîj¬FE@"(évј?ü-­$ß³?ÎRœ-Q?¯ÅHŸ5Û?ã?Ðà@ÿ'¸ÿ»b¿ç£æߝ‰é¿áÅâÝÛ<ý¿ïš@2 ?æÿOÁ^Y¨¿Õºt»=Ù)¿ÝÁ'œzIAGNbllRX J0712.3+5719?ïÿ'¸é&?öð/?x·oÇj?öð/?ïõ˜ã¼'Ž?UZðÆò?TÎ8Ï(À?UZðÆò?ïí*̀sO?o<Î&9Í?bÕ2<4Y?o<Î&9Í?ïþúïŸà†?Ä@\? Q3ÌҚ?Ä@\?ïÿ"GR¤é?tõø'þ\?·ã¥Ôn?tõø'þ\?ïÏÀ'g'?{Jí±k>à?xòd
'$?{Jí±k>à?ïÐà"—^?'R[8S7C?wîºÓ9?'R[8S7C?ïú¿û>`t?@ÇÂcŽ}?EÞ\Yh?@ÇÂcŽ}AGN4FGL J0712.5+3311¿ãéą38Å@2Žª:э&À;€y1DFÀ<¤ªIë@ #÷êï]?ÚI…ÚõÚb?ôj\_|gZ?îûÀÖ…&?ó¿hæsg@˜'°H1ȿ畟¿MˆI¿é¸;Ÿé¿îÍD¡š™õ?éÚFsBî¿æPÊï¿ïú'`åóåAGNbcuNVSS J071224+330953?ïò³ ~O¼?Ç…~ô@ž?Z™¿H·K?Ç…~ô@ž?ïó—ô¨ß?]ØF•H µ?YòÏ»ø'Æ?]ØF•H µ?ïdC^N"ã?	[x• ¸?"w"7å1Ž?	[x• ¸?ïüPÓÏm?7¼§ïHŸ
??½xÖúÀB?7¼§ïHŸ
?ïèAÉ谝?p"?"	q?g¾60"?p"?"	q?ï¿O^‹"?‡ýΥԋ>?€,=.ä`ê?‡ýΥԋ>?ïmç½Ðé?¾åüº?'C@ÕØñ?¾åüº?ïûZrx~¨?Kã+FÍõ?B–6.¶W?Kã+FÍõAGN4FGL J0712.7+5033¿ïZúXÁ@7Ý÷¯îpÀ9ʉ%®À<9M÷×ü@Oô**¡@wڎVo?¤)#~¤?š<&]#?ón_ċµ«@®B"ùF¨?ïÿH˒:¿Þ±	!ç±U¿ä)S€°"ˆ¿ã¥Ž/L¿ã{A–£E¿Øºùe²€AGNbll3FGL J0712.6+5033GB6 J0712+5033?ïþӖÚ;d?¸ZÔÙË?"Ɠˆb‰?¸ZÔÙË?ïö`^åh¥?VËJ¤?S?B'%õ‹?VËJ¤?ïòâ)o(ñ?Y(ëW攟?Z;¬³º™?Y(ëW攟?ïýÿbúT?!¸9à?l?0L;š­?!¸9à?l?ïÿ#Ý"?¡·ªBß?›…]î(?¡·ªBß?ïÓu¼€àv?wÁßž%?vE! £Hü?wÁßž%?ïêŸÃK¼?p¼ƒÁz?e`<ážÊ=?p¼ƒÁz?ïýjð†ˆ?*ªÎ $ÿ&?4¨~ñ¢Îå?*ªÎ $ÿ&AGN4FGL J0713.0+5738¿Üd…ˆë@9wt¼j~úÀ:ª‹#À<[AE÷@sáo@Î@Ãa	/T?µ±¿?Æi†?µóãqT?þ! v˜Ò@úÿý{ÁA?íjAQÙçh¿â•?í«À¿åÒ<öˆˆ¿ã£š8ûÊ¿éf\፿ïȶ`x'AGNbcuGB6 J0713+5738?ïýȽ@	R?#13:Æß?1ºÚSJø?#13:Æß?ïõ]OÄìâ?WJ圞|?UE`e¨Ú?WJ圞|?ïë3;…€ø?iÿ`aVi"?dÌÄaÁØ|?iÿ`aVi"?ïþyè¤CÂ?IñÕW§?(aqïÌÒ?IñÕW§?ïüc3	J?24×,Ðpœ?<çþ‹þY¡?24×,Ðpœ?ïÕ±<Îg'?x}ól:
2?u'a}ÿKX?x}ól:
2?ïã@žŸÓ?qžWû³ÏÚ?l¿bYì«?qžWû³ÏÚ?ïý?¤kì?'UÙ¬È?7~cÞ
Ô?'UÙ¬ÈAGN4FGL J0713.5+2537¿ïÉÄgu@/Ù¾ôœõoÀ:¹×†d2¯À<ƒÅg}¾@¦¾p=«?ýǝÓ[\?Ðú±AV¥?Ò—ÀÑkî@Ÿ¿ž ß?üë&¢E?ïÿHµ{wp¿¹ò4æ;´¿å±æÍ)¿Õð9Õó<¿í¡Š~ɉ¡¿ïçôpÄÜAGNbcuNVSS J071336+254016?ïÙª=«² ?iѸBžÚz?s*áG³"Û?iѸBžÚz?ï9%¸Ì9Õ?š{d†Y¤K?˜ÛHߙm?š{d†Y¤K?ïRžÄŒó?VKùؽ?Ÿµ¬,•Ë‰?VKùؽ?îAj°š^ˆ?‡
Kâaû?«éTóÆb…?‡
Kâaû?ﰎA‡ç?€E)pð$?ƒÜo¦ÜÆ;?€E)pð$?ëó.AB%Ñ?Áa¦Åôbà?À3Fú÷h¾?Áa¦Åôbà?îËe)áŒ?ŸTõèP]?®ÓI©dE?ŸTõèP]?èöë'*«?¬—"1ü?Ì$Q»UùS?¬—"1üAGN4FGL J0713.8+1935¿î¹ü>ïê@+'ãÑÌÀ8Ü#™b<5À;ØߑËnÿ@_""	"@-ÍbôÁÞ?ª";}üÒp?»	7¡¬ãx@™ûçl‹D@µˆMÁÔÌ?'%f ‡¨¿áˆÿ΁ٿå4ƒ•KV@¿åãÃb(¿ìçù¸¢ž¿ïúÈRꈟAGNfsrq3FGL J0713.9+1933MG2 J071354+1934?ïõü¦¯+Ò?P"ƒ€`·?T²é ;q?P"ƒ€`·?ïï≀$†?e
%'b�`vF"
+?e
%'bâ§?ï¦(ç»÷¤?'–óúu'?†uÆÀ‡?'–óúu'?ïÿ"íni%>ýŽþÇän?¨òPïí>ýŽþÇän?ïú&ó{?@òO[£"?Gg¿è¥?@òO[£"?ï¢æÝK+?ê"E"?‡FH¯^af?ê"E"?שּׂq›V?‰AŠíaöH?"þ"±WšS?‰AŠíaöH?ïÿJŸÊÈ?Õ§4ï¶3?¬?Õ§4ï¶3AGN4FGL J0714.4+1110¿Ò"@`º¢J@$H÷‡‹zÀ:Èû>ÐhÀ<rŸC@Ùî»4@¤XÍ?ÐÙ=^m"?ÃØáty¥?ö¡]b±¦@|Wt0('?ïýƒÿ("Ÿ¿ÝûÙ)Òa¿ádže0[¿×î,-…tI¿åŽœ`w	¿ïÿý¡UûŠAGNbcuNVSS J071416+110830?ïüž;"Ö'?68(4io?;"®ÞÖ·?68(4io?ïìñ¢g…?e£ÜÇj­?cú¢Pªñ?e£ÜÇj­?ïç43°¨÷?g^ÄÅ<A?hËÌ!ü1?g^ÄÅ<A?ïî.¾KY?@BõlÈSz?aÑAâ´¦Ì?@BõlÈSz?ïü«½²Ò?;~¡ÖƆ­?:¢d9ïE?;~¡ÖƆ­?ïs‡H€™»?–‹òŽ"±A?'é
°?–‹òŽ"±A?ï¿ÆוR¸?' žC
9?€Jå?' žC
9?」ѣB²?f´€ø{bà?€—œV½p?f´€ø{bàAGN4FGL J0715.3-6828¿ïÿxô(uÀ6øƒ‡ß\òÀ;i•ÅσÀ<xÉ7Ã@šh®ëƒ@môݍq?Ä<Dÿ¹^0¿œsY>	Ðä?Ø#"Øå@.`÷炱?蝷€µG?ÊOø{QZ¿é¥b$¸F-¿áÖ3ž$E¿âešŽŒ^¿Ð~Dß-!¡AGNbcuPMN J0715-6829?ïýó…ô N?'¿Ÿ'ôA"?0cÐ.œ«C?'¿Ÿ'ôA"?ïôå:´?ViÄìÚR?V5‹Å‡»?ViÄìÚR?ïí?ö‡}°?d‡ÒjóV?bÀ	eD€u?d‡ÒjóV?ïûaú_ÆÔ?)}SÀ·?Bx](Àå?)}SÀ·?ï÷ÜZ¤*?QŠXê˜æ?PGӇ½ˆ?QŠXê˜æ?ïÖfðé¦f?x÷#‹i
÷?ṫ~I?x÷#‹i
÷?ïÓµ‹Vy£?~ÉøVVw?v%:lÐrP?~ÉøVVw?ïäü@þð?[àכZØt?kúéœ7˜?[àכZØtAGN4FGL J0715.6-4528?äþi°{fÀ.
_V§¬'À:.ÄBº³À<S"}¨¢K@ïE…pB@=Uæ¼b?¶šõº¿rdœBÞz^?¸"~!™ï@wNö³%1?ïõÄr‹7׿äãü":µ¿ä‡.]
¿åÓPÊï¿ëüœ#·•?Ûáad°AGNbll3FGL J0716.0-4525SUMSS J071544-453031?ïö¶n'ƒ?bh¦ùá?S"uS™N?bh¦ùá?ïöŽ£hÈ?WgŽÄ{\ÿ?SÆâK:ñ+?WgŽÄ{\ÿ?﹬bã¾Æ?ƒÙ¦h †?"ç8Iü°?ƒÙ¦h †?ï÷Gäèná?=š^¯¶öj?Qp6<ୖ?=š^¯¶öj?ïތ
mtÖ?hÝP
@¨º?p¹úÒä|ã?hÝP
@¨º?ïÙ¯d9Ãú?y×»Ô/)?s(NjW?y×»Ô/)?ï›JFI?ŒiCì­?‰-nqN*?ŒiCì­?ïáåø?Æ?^î…zBR?n¢:™Û?^î…zBRAGN4FGL J0717.7-5519¿èÁl¶%…9À2zîÇÉWÍÀ:õÈ	ïmÀ<ŸµV¬µ@ úÿ£8Ô³?÷´º6È*?ÒÉu)wȎ?ÞÁS<=@âݽµØ•@·a·?Ôúß?ï]'îY¿äÎ˪Þ?µn˜K»À¿álN']‹¿êÜUÁR›-AGNbcu1RXS J071745.4-552024?ïøÑɍY?Fò»Ò×[?L¸ÛqxR7?Fò»Ò×[?ïÁÌíô©?…FW‰F?üyçcX?…FW‰F?ï–}÷Á[ï?€"bìí?Š`' 0?€"bìí?ïe3›å†?x͹G9ˆ?"YŒ…¬IA?x͹G9ˆ?ïók»˜{?V+Vé›b?Yß(Z[?V+Vé›b?ï*Þ/B/G?§'RRˆ8?š¤:á?§'RRˆ8?ïRôÇ<¿ú?'ÉàÁóÁ3?•¡gÐúÑ?'ÉàÁóÁ3?í¢óá
Ì? "ÐgN'\?²ï`÷'œ? "ÐgN'\AGN4FGL J0718.0+4536¿éêOy1f¢@7tàP7PÀ9ÃJZ—%KÀ<G'ñ·gá@Ls 3&@û¥»ç?²°Õ_îR.?Ì-˜ªwŽ@o1'Y4@*€='(?ãRâ/àm¿Ò]³ß@¿ç4~!nÑ¿ç ÐàWÄ¿í ìt2¿ïúöv'"AGNfsrqS4 0714+45?ï"Ól¼?ƒ†¹¹
îü?e——2w?ƒ†¹¹
îü?ïîÑd¿¥Ð?dEVf3$?a.›3û—ª?dEVf3$?îk´ÐÆpV?™]–<òï?©D²ñá,¡?™]–<òï?ïï´‹Q?Ej6Þý?`Kô³»?Ç?Ej6Þý?ï3ZSQ?'¥Ž?Tpô?œY"·UÃá?'¥Ž?Tpô?ﰃø¿ç.?1@Áp‹?ƒßà,^ƒ?1@Áp‹?ë¤÷Üù?ªê>²I?Åo´ Œ?ªê>²I?ïº{Îp8?i•pž²_õ?arDº?i•pž²_õAGN4FGL J0718.6-4319¿ìÓÁZu8ßÀ+OíA·ZuÀ8œT§!A™À;'³ k°@ß¥ídó?ü¨J¡äÁ¶?¤Ÿ¨@?O?¸‡žß–ä@€€B_@´ jÓ?Õá¼'-@¿Õòâu«}È¿Ý÷:Ÿ
Kî¿ÕÚJ¤>
W¿âŽÌ¡ƒÈÍ¿çÈ}GS{¨AGNbll3FGL J0718.7-4319PMN J0718-4319?ïÊvø¤R?'5ø®Ö®T?zÄ¿k½?'5ø®Ö®T?îË7
z¤®?¥N9¡5?£LZéj?¥N9¡5?îþý$ÖØ?—PÃìó@¦? (Ö«‡?—PÃìó@¦?˜‹5?…Ó'qî`Å?¦u¶'¶è°?…Ó'qî`Å?ï®kÛÖ?™p•àN?œŠ2"Å4?™p•àN?ç4C•šË7?ÎèFù—8Ê?їxÔÊi"?ÎèFù—8Ê?ﲏÅìo?—M¶¯8™"?Ÿ	®iÜ?—M¶¯8™"?çÔ~bd+×?¯¯òzf?ÐW;7¨R?¯¯òzfAGN4FGL J0719.1-7055?ìèLÒcÀ7R™ú©vÀ;Ø©yámÀ<£Vh•ì@ '—)§Ä?ýá¥Ãsˆ?Ìý™ô2ld?ÊáYv¾Î1?ý§Ww¶@`õÏûUv¿Æ¯h¸P?ïÛ }-¨? 2=ûõ?™¿Úoø æ¿ç;Mlš]¿Îyz?a>ßAGNbcu1RXS J071910.3-705411?ïû´™z:?4ñWù±É?A-š˜ICà?4ñWù±É?ïêêâŒ|¦?c°ÕóDØ?eAÊU?c°ÕóDØ?ïàó'mâ?`°ygŽÙ?o€H}ô?`°ygŽÙ?ï¯Gs刎?eí¿b`ZN?".#Eæ}?eí¿b`ZN?ïõ¤.?zâ?P#ì<éûÐ?T·£ËAÌo?P#ì<éûÐ?ï±ìŽß?‰‰T^g•?ƒ"Ü8µÕ?‰‰T^g•?ï«f¯ô?"q¿Ö4M?…?ºm3;?"q¿Ö4M?îÃã;	?±IF?£ÁÏó¼³w?±IFAGN4FGL J0719.3+3307¿îzl¡O+È@3Ü£}™‰À8‡Á*[À;§Ü®ÂË@1<¢ô@¨l›3͍?œRiH1á¾?ºctïk2S@ 4çhY†@cÇ8ä")?psecÜô¿Ýû÷|ù¥É¿â­½½æ*¿ä0Ž]{[@¿çTèÅP׉¿ë`B5ÃAGNfsrq3FGL J0719.3+3307B2 0716+33?ïù¼.*F?IŽ ®
&?Kõ†ìÈà?IŽ ®
&?ïØ|^Üj‹?Šm²÷=Ù?sÁДŠj—?Šm²÷=Ù?¦Õ%Ў?"
håJà¸?€ÊÇ	üp?"
håJà¸?ïûÄâXá?6þ5;/7¤?CøëƒŜ?6þ5;/7¤?ïîB'0œ?`	¤H†n?a뽄®›¡?`	¤H†n?ïF&˜ðý?®;!ó}5?—=Û.™®X?®;!ó}5?ïÏÚ
ۓm?ƒl|)'ý?xùuY™?ƒl|)'ý?ïé†gžÛß?XùìÜ\ðÅ?fy˜2iqL?XùìÜ\ðÅAGN4FGL J0719.7-4012?æ×$ˆ9dÀ(VȒ«hÏÀ9¾Ò–³5À<ºö
³¸@–R½<6@x+h{?¶é±4v?®ò«â$*Š?öê¹aµý}?÷HýLœeÒ?ëG†Â&€¿ãr
™E¶Ã¿äÑ[ý¬¾¿ß ϧƿäퟫ+'U¿êi>]ˆÇAGNbll3FGL J0720.0-40101RXS J071939.2-401153?ïø¾BEtÔ?Aåq?M÷t)Ë?Aåq?ïµ/ßì5?…ÕXo?'´Ü2Æ?…ÕXo?ïψgÜÌä?u9Îí¶?x;Ëôê8?u9Îí¶?îÔª;IÏy?†Fn ‡m?¢µ\NÒ¤g?†Fn ‡m?ïì¼ÐŽ?Xùa¶ïaí?cC/ë?Xùa¶ïaí?î†l
¢Þ?¯¼¢s	v?§Ÿ‰=n?¯¼¢s	v?ï¡ÿTðƒq?†SJãz¤'?‡€*Î-÷"?†SJãz¤'?é°æ1¢ºU?­ÃÉäÐ?É<g9u­?­ÃÉäÐAGN4FGL J0720.0-3507¿çþã%ÇÀ#ÈîñºÂßÀ: žóu®À;ýPMö-@ѯJ/ùî@økú$ì?½	§ž•?ˆ1È=à¥?ËnÞÅr»^@©èsFs­¿À"dÌ2s¿äK G2Äx¿éïa|¼¿äž{`sˆ8¿à'ª&¯—2¿Úk	Cº[AGNbcuAT20G J071959-350448?ïþ¤·ÉŸ5?¿BbÞ?%´…/rL ?¿BbÞ?ïõ}ÎV?Vèg¯­?UÈvÒä?Vèg¯­?ïä[kP?xÙ's–a?kî¤ÊºwÚ?xÙ's–a?ïÿƾã!š>éJ§X ¿ã>ü ‹b©
>éJ§X ¿ã?ïþ,RM–?+Bþïqâ­?-:à±Ñë˜?+Bþïqâ­?ïËùOrë?—g"¥!?z}@9F—?—g"¥!?ïÊzG"ñ?ßýK-ǂ?z·Æ8‡©?ßýK-ǂ?ïÿ9ôýk?ž¤('h?ÁxD–¸È?ž¤('hAGN4FGL J0720.0-6237¿íZâPäìKÀ4¹"åûqüÀ:1SÃÌsÀ<40i@µ—;ÆU@¼›"Ud¶?ÇWèߧðÊ?Ï5E‡Á?ý5Y~ —@›èñƁY?îó‰p"¨¿èyÂÅâοí5#ÞV¿ìÌJ@•òE¿ïÿv}_Ò#¿åÅ2à'AGNbcuPMN J0719-6218?ïø-[¶g¹?PlØaXc?OJ'Ÿc£?PlØaXc?ïæ÷z—Ã"?ó´ÂeÓ?i…R?]þ?ó´ÂeÓ?ï_`átØ"?2çÙ¤"Ì?"ãÓÉÅ?2çÙ¤"Ì?ïàY﵅?YùÈ	æ?o¦%_0¢?YùÈ	æ?ï敖Ô?ioFîÖ©Ç?`ãV)Ü.?ioFîÖ©Ç?ï³Lð7yÙ?ü¨ß<#?ƒ,Ãý IÈ?ü¨ß<#?îƸQ\?—z{ð\(?£"zð½ëÿ?—z{ð\(?î܏…Y"?'Âz?_‡?¢7ib4Í?'Âz?_‡AGN4FGL J0721.3-0222?¿ê
¢#	@2Üû:À:ØúåäËÇÀ<b7£Û;û@!
ÂFá'?þ-î \+z?Æÿt>ì$?mWtárÏ?"VdnÆ@[Ž(¢5Ÿ?æþåþ÷í7¿îÏ
)N­ã?ØâõãÇe/¿åQ¯õüpÿ¿Ø©`Ó)ˆ¿À°{±|9AGNbll3FGL J0721.5-02211RXS J072114.5-022047?ïöH±/d?… ÚŠãcá?Sn¯åH·?… ÚŠãcá?ï뚖ªâþ?sfäóڌº?deiƒý?sfäóڌº?ïè$pïùš?v{ ¦ù\'?gێތC?v{ ¦ù\'?ïùƒÿJð·?3Ï${¡G&?Iðƒœh2?3Ï${¡G&?ïü½ã¥×@?5gÍÏÌþH?:ä×$º?5gÍÏÌþH?ïTXGrbý?¤*ÿWðt?•t÷	š|?¤*ÿWðt?ïònís‹h?p°ŠÞ«š?["$'8€À?p°ŠÞ«š?ïðxÆ\¾?QŒ²L6C?^åAÌ% ?QŒ²L6CAGN4FGL J0721.3+0405?â×3€`°@!.3ïñ•À8îH[¹d:À;Ö@&t@™`ùj½@}ÝÙdŠÄ?­Ù=ôWUQ?ÀtƮЍ@u–AöD•@à‹†"¿Å.ld'5¥¿äÊf¿ç5ם‹@»¿çÿ©-‹S†¿í¡#›æzô¿ïÿç<t%AGNfsrq3FGL J0721.4+0404PMN J0721+0406?ïö`ÑÉXF?I€9æö'Ÿ?S>[ñ…š?I€9æö'Ÿ?ïáÝ¢h¸?xÏpý)r%?n"]Iˆ?xÏpý)r%?ï»H
"o?v¸¶#—?-ü•üÑÙ?v¸¶#—?ïêàžÏF?O2Dôe‹?eaKtʏ?O2Dôe‹?ïöNó>b?Qà™%Û3?SÛb2@lF?Qà™%Û3?îô|h<ö?¬úÌõ-í? ¸9{̜?¬úÌõ-í?ï¹L¾¶	?"	îô…þ?¬þ@Ü?ç?"	îô…þ?ï‹xl8?y˜ÇٓDÄ?>!ëæ'%?y˜ÇٓDÄAGN4FGL J0721.9+7120?롆¬SP@<»à~íÀ6CÀ:Ð{?;2@e°Ñn?ÿÇ@ÿ¤?'AçÅ?­ÄÑ<w•@"¿U›=È@§6ÀÁ&¿¹.CŠCeZ¿Û3ÀîÈ¿âJ'Û¿à£W±—½¿å›aðµà¿ä1Ÿµ<OAGNBLL3FGL J0721.9+7120S5 0716+71?ïåŒf!¿e?"ãt϶~?js™åÓ%?"ãt϶~?ïßÀdï?€íéwßQã?puŸÏ¼3?€íéwßQã?mÓ?'nn -½?Þ{h.§-?'nn -½?ïøüëoòy?Cáé©©?LR,øM…?Cáé©©?ïì·×Oæ%?`'DB-"?cH(ì'úÁ?`'DB-"?ïn(¬hö†?¨`#<	(?':êq)aC?¨`#<	(?ïւÒó?'î¦= ?t¾–áÕÞÉ?'î¦= ?ïè)Þ[ü'?`‹ßö¸í?gÖ!à|Že?`‹ßö¸íAGN4FGL J0722.7+3606?ïð×uÆE@5ZÀ?öÀ:¤p¼*¾À<xåÈFUO@æ‡ÒǸ'@ـõ]åŽ?Åã!wôÙ0?¸ÔÈnÄ-í?ðdåÈFUO@º8	0Ö?ï—ùá­Ún¿Þ—¥ãÿÄF¿é¿8ÇǪ¿á)Œ 4Rî¿ïý
í™Ëï¿àIí>²B]AGNbcuMG2 J072255+3606?ïìsl¼Ê?†+ïý;?c茡¥™?†+ïý;?ïðæ£?`'á¦ÄN?_ÁáŠ<»?`'á¦ÄN?ï×>Y›Á?u+c<ܛt?t`Ó"ÿÂ?u+c<ܛt?ïÚ|Ãu
C?Tvü²Ûä?rÁž4ü¾"?Tvü²Ûä?ïäšmmÛj?l«Ñ)¨ÅÜ?ke'Ê~.%?l«Ñ)¨ÅÜ?ïÀôŸØ*­?€6ÛÿÎ?…° IA­?€6ÛÿÎ?ï¥ç'…_6?…w§]OÜú?††éˆ?…w§]OÜú?ï8G«Kƒó?€õÚóŽ%?˜÷
"׳ž?€õÚóŽ%AGN4FGL J0723.0-0732¿ïSò"äVŠ@_9K{)À9äٞlg1À<±KgŸ@,­†¶h@°››ÒXþ?ºu…NQ?¡£0P¾^?èÍm¦Ìˆ@º	Å{ ?ï‰>½ªðÚ¿á{0f…p¿åÅ$aß¿áKñpD¿àÈ.3ïò¿Ù¬¾Å"3‡AGNbll3FGL J0723.2-07281RXS J072259.5-073131?ïòjÔgÔX?rà?‰m}?[*W…Ÿ?rà?‰m}?ïÜ(h­!?'€$ò@ñ?që̇?'€$ò@ñ?ïÑQPwB?~…±Õ¯…M?wWWÌ.?~…±Õ¯…M?ï㨛ë˜?Py§ÇÉ?lWdXU¿Ã?Py§ÇÉ?ïã:*¯gG?c>±·q?lÅÕ? Û?c>±·q?îäNџD~?«£•Édê9?¡»ãx?«£•Édê9?ïŸÁ{àÌ?‰º¶é™]Ë?ˆ ý~*?‰º¶é™]Ë?ïŒ3·Y?uPd"ÊÅ?Œóßè/?uPd"ÊÅAGN4FGL J0723.4+5841?ÛÙi=[U;@:ÿyB=À;å¼i¨:FÀ=¾@Bo@"{é~^TÊ?í@*ýڋÒ?àfQÒ[?æÝñLÞÕä@È¡#і`@a«ã=?ïÿõÿ 1#¿ç²›"nÝ-¿ïÿÝÀåãÊ?ïý¸Ý¬˜û¿ÁSIÔ	'¿Ø=ª]yAGNbllRX J0723.2+5841?ïñ̼dRn?`R·	z}Ï?\f‡¢ŽôD?`R·	z}Ï?ïò®&"6?]×hʀT—?Z£ÌLóà?]×hʀT—?ïÿ7¿E6?‡ÀÅ*â™Í?ïïH?‡ÀÅ*â™Í?ïø_"ág ?E¯c´,Ä?Nƒtèá½i?E¯c´,Ä?ïß;þov?uÀrrJŒ¡?pbªç¡?uÀrrJŒ¡?ïÊÝøiS?y'ʀ¡Ž?z'ªý«?y'ʀ¡Ž?ï{&eßÉ?Œ:›Fé)?›3EÔTé?Œ:›Fé)?ïè4 1èt?jHŽçrk1?gËß¼9"â?jHŽçrk1AGN4FGL J0723.5+2900?â
lÿ@3AƒÆÉ}À:¡4êÃWÙÀ<h"»@}¾ýVW{@iüp?Ð#þA¹Þ³?ÁfbÍT²?ñk:á}^@
¤ý·PcÆ?îáßeUÅ¿ãô®ÞOV*¿ãôC¾ñ—Ý¿ê~è=k›Z¿ïõÉ{´Ú¿ïþI¡ßŽEAGNfsrq3FGL J0724.1+2857GB6 J0723+2859?ïýØ0`΀?(æ¯)f?1>}<üý?(æ¯)f?ïôŸÃK?WI@æÀ?VÀÞÑ_ð2?WI@æÀ?ï݆/hµ?líSJö¾?q<èoëÍO?líSJö¾?ïøR-Ž}?5_‡XI"£?N·I‰ût?5_‡XI"£?ïþ`D۞™?,'èÃg²[?)û±ô¹Gh?,'èÃg²[?ïË|‡(íy?€mÆ/ˇ?zA¼]ç¨?€mÆ/ˇ?ïφ°³¼†?«§½Ý'?x<§¤ùB?«§½Ý'?ïæMÊÁ¸O?TËC³ÿŽ{?i²5Xd¸—?TËC³ÿŽ{AGN4FGL J0723.7+2050¿ì@½È«ˆ@07!-w1À:Zڀêv+À<c" ³Ô®@ £ˆ6šÆÀ?ÿkªs±?¹*Â÷6ð¿¡xô2—Vô?ç:ê _@ü°­\o¿ä›?î¿åôi"PY¿âA¥¼½‹¿ÙɱÅ	‰ì¿ãêÿ½ºá?sKç¢ËAGNbll3FGL J0723.7+2050GB6 J0723+2051?ïüw*ÀL?-ɂPí­?<F«fVwø?-ɂPí­?ïñcՒn,?_É^©¾µÊ?]8U^÷l?_É^©¾µÊ?ïôe¾±è+?ar!Â\Û?W4ƒ"àXÞ?ar!Â\Û?ïôõ_èóÊ?>䃹ÎI?V?º¥ŒÓ?>䃹ÎI?ïøL€>Ý>?C$s2©¬?NÍÿÃÛ­?C$s2©¬?ïÃTb¥3"?ƒqïƒsy?~UιÓ?ƒqïƒsy?ïù
Ú«?ap³Œ€÷¢?KȔ|(Ã>?ap³Œ€÷¢?ïËê΄KÃ?iA#ÿ–%)?z
˜Ìøf8?iA#ÿ–%)AGN4FGL J0725.2+1425¿ë"àD±á@+Ó"Àh¡À7ÝàÇU•À;‰¢TS>k@4#.XX@ —Œ™?—ÄCøc®?°²œøž¸@AbÙ,@¬¸ú²ä¿Å"V¼OQ¿áfÕÂ>ÔQ¿äËj—MŽÿ¿ä
оsæe(]í!¿íƒá¡p'°AGNFSRQ3FGL J0725.2+14254C +14.23?ïû¨uˆý?=¹ ;º±‡?A^*úk?=¹ ;º±‡?ïìû§÷ß?t^áò¿?c÷4L1`?t^áò¿?ïàÐtn‰B?wyŽ^ïxð?o/‹b¼A?wyŽ^ïxð?ïÿ͂Õ1ö>ð!ÜÀd¸>ù>|œp'>ð!ÜÀd¸?ïþ}P… ?!ìße¾×¢?(*øɬ?!ìße¾×¢?ï"#«€ÌÄ?E¬lQ?Ž÷ÌÎû?E¬lQ?ïîû¹|ìm?qsÃÄT÷?aFº
RZ?qsÃÄT÷?ïÿ¬Z4C?Ùâ<"ó?û zFa0?Ùâ<"óAGN4FGL J0725.5+0216?ØÄÅ䝛S@!AlÅûø4À9Ò¹
x)À<ñü1>f@
Â
|?ÿ1³¡'œ'?ºÇð-"£?³¡ö4z0?úqºÝ¶ÿÜ@ÑîøEÌh¿àã£=‡J¿Æ(G‡S¿ßøÔ<­°R¿áAn?"՘¿Ü/0Åпæ%Pò`ÛAGNbcuNVSS J072534+021645?ïþYôVî=?°øN'?*`½`0ÐD?°øN'?ïëJêñW?p\«qDP;?dµ*q‰(?p\«qDP;?ï÷E·\G?>Ç»¡Í‰?Qt'èÄPÝ?>Ç»¡Í‰?ïö©sÆ2?6"'Œ!f ?R­Éë?6"'Œ!f ?ïü¢{H(k?0îCRWÁ(?:ì&o—?0îCRWÁ(?ïYÀ"~¼?žËŠXâá?"Çþˆð™?žËŠXâá?ïðS«‰í:?lžCiç?_X¨Ë)K`?lžCiç?ïßN@nŸ?]B%õ¡?pxXó¶lu?]B%õ¡AGN4FGL J0725.5-0504?½ ˆK=–@í:>À/0À:Û_D35·À<BxÔ'4!@!THÈpǓ?ÿ¯®(œ×<?Ãs…]Íf¿Ÿ¯¹|Ê?ßÿ^¢Í @aW<|Þ?ïõub'¬¿ár"›R×=¿ë*:э%î¿Ò¹'"µí¿åµ(€Ò£P?™òåæ#`AGNbcuNVSS J072529-050338?ïüLÚ-Í?6‹"°PF+?=ŸÁ¢uÓ?6‹"°PF+?ïãBî<3?s01°ƒf?lï¼ã	
?s01°ƒf?ïí¯Š5'M?T"[+æ1?bPu–3£f?T"[+æ1?ïé½'µþ?Khç_ž?fBØY€Ip?Khç_ž?ïô¹àXgB?XIÆd×?VŒ?·¥œ%?XIÆd×?ïN|vy?¦¡´™âÙ?Ÿ60j`X÷?¦¡´™âÙ?ïãE«õ€?s1ðR	ûh?lºSï'1?s1ðR	ûh?ïwäÔçŠ?}…]'ÈxÚ?'CmúÀ?}…]'ÈxÚAGN4FGL J0725.6-3530¿ïª>°tÎÀ"gn¤"ŠÀ:Åõ´L£GÀ<!6ãÁÛØ@ 0Î"oO@Ãlß&k¥?Äí&ο ÏÉ£Äã?à'qßÁ@Fx	|?ê'ݝ'A¿èæT]Of¿êýÑb]ÿ΁¼ÙÏ|¿à'8¾né¿à:Ã_æš~AGNbcu3FGL J0725.8-3532NVSS J072547-353039?ïþ­ó¡Uƒ?ë²îÝð?% Ç¿"'?ë²îÝð?ïöÂÙü-?WÀ¥ª§'ˆ?SôyæS71?WÀ¥ª§'ˆ?ïóÍ‹­¯?[&èëõ·?Xeʀ0'Ð?[&èëõ·?ïþ*öE?Q'?£¼?.MTZîã¡?Q'?£¼?ïüi#j?G<‰(ÄxÅ?<¶æ €?G<‰(ÄxÅ?ïÏdÌÞ?'?ƒ¹—%ù÷A?xM™–_—†?ƒ¹—%ù÷A?ïçocÌ>n?s-"¢Ð'?h›üÇҗ?s-"¢Ð'?ïõXq'¬å?J—:÷œ?UOV6?J—:÷œAGN4FGL J0725.8-0054¿ã&w9-¯L@ñµ ÝDÀ9@†ºŸ¤À;ûbqåª@k¶ÓfD@£ì¤©(?©¡ÛÝ`î­¿"Fù¨fÕ¼?ê':…7@–¢n5é¿áaÂÈg¿áµ2Ùà¿âíp3Sê¿ÜŠÛ»¨N¿á%_Ö)lá¿Ý×_¢ÒÓLAGNbcu3FGL J0725.8-0054PKS 0723-008?ïýÌ_MÇ?0ßਚ?1ג¸G?0ßਚ?ïí¡C1-?jÙ(—ý ø?b^½ŒQ?jÙ(—ý ø?ï÷
òç›?`—öWÅM?Qê]÷Éz?`—öWÅM?ïøá§
¬"?7Ü¡)Áïæ?LycÕÚrÉ?7Ü¡)Áïæ?ïû ?®ŸC?7vÍq˜ì?A«né?7vÍq˜ì?ï[¿>ê]?¢-¬?ë?"ˆB
d?¢-¬?ë?ïø?5V'?`=û{eh?O+WPV?`=û{eh?ïêÙaÒû2?VçOÂ!ƒw?e&ú*–À?VçOÂ!ƒwAGN4FGL J0726.1+8114?æ––b‹@<ÊÙ­…àÀ;çè:ç\›À=#Èb±@!r˜k?ûkëšî-?Ô)|»'gÌ?Äseè½O?ð<÷ØQì@‹cöÊw¿ïÿÿ)@k*?ïÿˆ¬Œ%?¬,©ßÀx¿Ú"s,G†§¿éôœßõ¤?ވ^Þ²¨^AGNbcuWN B0716.0+8119?ïøVÉx?N>ÎÏØÿY?N§ßË\Ÿ?N>ÎÏØÿY?ïퟴL¨?m'¢a¹¸Y?b`Kޒn?m'¢a¹¸Y?ïk‡ ÑNð?Ž¥9,há?'éE½õ?Ž¥9,há?ïÏÈE‡&?aáuIÜÚ?xqùi8­?aáuIÜÚ?ïæ²2±i?eºhV¸–Ý?iMàՍ¦Ÿ?eºhV¸–Ý?ï¸cý^?Ž¯Ì|+j?ú&ö°?Ž¯Ì|+j?ï½UzI·?"1‹ý£ù?HUIב+?"1‹ý£ù?ïAêÞ/e?‡}úôÖÀ¼?—¿'©¯j?‡}úôÖÀ¼AGN4FGL J0726.4-4727¿Çú"«uå
À,J ÊæBÀÀ9$ü!N.aÀ;ÂÁÀ)P[@T!¾@Âé@?Ä;-Ó?°s‡Ù~?¿úš ¹D@@a~ @Xj1Ϳ΋ÜÁ¸r¿ä•¤ýzꂿåÍùƸ¿çŏc}(¿ë—à±Ü¿ïÿÿ" 5•AGNfsrq3FGL J0726.6-4727PMN J0726-4728?ïúž!œ:'?:䌢Ϸu?E‡x¯U'M?:䌢Ϸu?ïóŽ4¼±?[ã5®0?Xãß9=È?[ã5®0?ïÊÚºm?p4Ÿæ*e?z'ñ4iÏ?p4Ÿæ*e?ïúmz½ò{?0‹2å ^è?FJ*)?0‹2å ^è?ï÷•>QZ¢?J*szin?PՃRKü?J*szin?ïƀ'ŒŠ?—Êqï)Ŭ?|¿¶ÚK?—Êqï)Ŭ?ï°X¯2vä?…Í9»ê?ƒéÔ;¡VÕ?…Í9»ê?ïäJ5"r¤?Zj¨0[u›?kµÊ®å³/?Zj¨0[u›AGN4FGL J0727.1+3734?ڟåtIº@6Êÿ:Þ"`À;Á­!5Ú­À<é°¤xí@!À?ÒþÀ?×fxÚÝ0È?èùäÝå£Þ?ïûÙ_'F—@~†T@wUCÿ3Q¿ë?.Ö­ ¿ë¹‹§i¿Ð'4è¿ÙcÍÚ¾Òä?¾°»Ê²¿ïÿýFKêAGNbllSDSS J072659.51+373423.0?ïóÇðÄùš?hX¥òÅf?Xpï\R?hX¥òÅf?ïô£xjŸÜ?TñMI¡™?V¹ŠõW?TñMI¡™?ï^MJ-2?Ž4 ¼:¾?"6V¼çÅ?Ž4 ¼:¾?ïùÌ£mi ?=	*†¯úC?HÍrûØÿ?=	*†¯úC?ïëThHO
?n0£ŽøoU?d«—Êîŀ?n0£ŽøoU?ïÅË9\K?€øoq‹¶=?}xÜr¢®?€øoq‹¶=?ïrîþŒÁ?5·‰þøÂ?'¢ 1ëãÓ?5·‰þøÂ?ïöfKl?[Â¨g&?S3ja,öš?[Â¨g&AGN4FGL J0727.4+5325?çŽÈw@:²v‰ÊÀ:íâXOLÀ<˜V>Ðö'@'èZÔ@ïd†'V?ÊJàc'†X?ÄO3Cú*Ô?õˀœ?üåàaª¿â Aåþw¿æ½£Ï}5¿çFÓ#(¿æ~'bEo¿ìmå€ø¸ä¿ïÙuQ»´wAGNbcuGB6 J0728+5325?ïí g(®?bB¬fK?bߘÜÑ@ì?bB¬fK?ïÈãä‡\?…MƒbíØX?{ŽwŒ\yè?…MƒbíØX?ïªIÁ%_ò?{›ÈVq)ý?…m¥y÷"?{›ÈVq)ý?ï"«û_Ì?rsœÍ[3?ŽÏTý¸q?rsœÍ[3?ïàð•KM©?jigÊ*
_?oj³R`?jigÊ*
_?în©›z?²Cj2e?©n)½ä^?²Cj2e?ï^Vø_M?•šE¬€¨¼?Ô5<Hj?•šE¬€¨¼?ë€Ü5—ÞÑ?ªV&֘"'?Áü) "½?ªV&֘"'AGN4FGL J0728.0+6735¿êsHìáL@<e#'Õ€À:D6•¾BÆÀ<vî>6œt@38¬nÞZ@ñÈ`2p?¾š%@èc½?«Ÿ!ÃÊ¿?æ†DhÜ
@`«fuªÒ?ïV*
ðƒ‹¿è…H©¼ýL¿ë&àtI}ø¿íecœ‡Š£¿ïÿž{€©ß¿ïÿÿÊPËAGNbcuNVSS J072854+673225?ïÖÿQj'?­­SUD~?t€W0™÷ø?­­SUD~?ïë
Q+…"?id)oÄïÃ?dõ®´Þ…?id)oÄïÃ?ï°ÄÉH2õ?ƒ]'"]çw?ƒÎ͸BÊ?ƒ]'"]çw?ï«Ž'Ã?rΞ—?…?8¦Äã:?rΞ—?ïɆ*ôAÓ?€q?‹ÅÁ?{<ê|ðw?€q?‹ÅÁ?﯆JôV?…™Ø—?"1brl?…™Ø—?ï pn¹,m?‡â|çü?‡ãäU$€°?‡â|çü?ퟬe®N?¡­}_ÓÚp?³œ×*Œ?¡­}_ÓÚpAGN4FGL J0728.2+4827?ïòQs»
³@9Òe8hýÀ:´w
}—À< ÝÆT@Ÿ1ƒZ¾@'Ê<ϔ'?Ã;äI·¯?±êÄÚe?î5r£‹‹@yþô'9¿âwÉЙ
(¿æÂ
÷9‡á¿ÜZ›âŸ¿ä &æô–?¿ãø?"û'¿ïô ÞÇÌAGNbll3FGL J0728.0+4828GB6 J0727+4827?ïø‡'üô2?i²Ä–ÍØ?Mã_QÑ6!?i²Ä–ÍØ?ïôn®Öº?V‡ùtÒ»%?W"¢§ÂIº?V‡ùtÒ»%?ï܂Àö;?xÕ½‹ W?q¾Ÿ'Ò°Ï?xÕ½‹ W?ïêÔw?G>ª$²Ê¦?e+íQy/Ç?G>ª$²Ê¦?ïð|¥u£y?U÷u…NÇ+?_´±ÄN÷?U÷u…NÇ+?ïÍDp67¹?{f-ÍÇ?y]ÇöÂE?{f-ÍÇ?ïåkgŠ±R?wH¶D ž?j"˜q/&?wH¶D ž?ï"ã|f­ß?tx¬· ?ŠÇ ð£\4?tx¬· AGN4FGL J0728.5+6128¿Ô0w@;ûd¾ÆyÌÀ:b]¶ŠkÀ<üýíI@%DĀ"$@\»‡*+?Ãe4b2O3?Ä´ú<ü¶?ýR;×F£R?ÿ®B0èU¿àtéa#q¿áÌ{n5gÁ¿éޠ4¿é'Öt{'¿ïï{ÎRß¿è!^™HAGNbcuGB6 J0729+6129?ïå·oËóg?i¢(¬ ?jH1Lég?i¢(¬ ?ï"Zseö?'ôe ?Šéy°äò…?'ôe ?ï¢ËàfÁ?x[ó|Å<?‡Mù&O©?x[ó|Å<?îü#Æ/?"ÿ$pŸ:È? =Ýã¦?"ÿ$pŸ:È?îî˜t*Ÿ;?†x‹c?¡x¾1óP?†x‹c?ì™L½Ñdë?Áa¢ýpƒ¡?»5štØ«?Áa¢ýpƒ¡?î¯Ôeê¸?¡²¥¬'é©?®•¹¡T'?¡²¥¬'é©?穞n ?¶ýÿÇ6e?ЬÃÕ#ÕÀ?¶ýÿÇ6eAGN4FGL J0729.1-3131?ïðѱôÀ<¹½üOqÀ:CTY©À<Wۉ(2@RG[^JŽ@À'¢Ü?ɸàœ7ƒ¥?¾JÍْ-?ðEUDÖ@JSÆP±É¿æ-z¿âp Ñò&¿æQøàüڇ¿ÝÝç;ãÛÝ¿ïþ¸Ø#B$?ïזàÜAGNbcu3FGL J0729.5-3127NVSS J072922-313128?ïîÅQr'T?[ê¾v?a:®À²ä?[ê¾v?ïðºoÒö²?`*ôÆtË?^‹ xO*ã?`*ôÆtË?ï°Ï¯fp´?€ØÛm3h?ƒÌ3ÊM
?€ØÛm3h?ïñ6æ"iÌ?J̙ô^xû?]'3e7v?J̙ô^xû?ﯬôrá¨?‡KæÚÖU?"Âð®
?‡KæÚÖU?ïƒnqD2V?¡7JIû?$c¡4ú{?¡7JIû?ï	Sò£j?šRúia?žÕ´òü¼?šRúia?îãh?'B
ñ}‹?ØĊ…•Ü?'B
ñ}‹AGN4FGL J0729.1+5703¿ïì|™ÈWa@;'ýq?À:¶nÒE²'À<—…\˲ñ@V±<£@ƒ¥An?ĝ•½ ~?¸Ø›ž<Òª?ñvÙ*© ö@ïéW•?ï¼ÊUú˜¿ÑÛiþKtó¿ê=7˜ól¿ßJ(B>hñ¿í­ÞA¿=¿ïø#'¬?AGNfsrqTXS 0724+571?ïüFž8Ô?4"P‰LEÜ?;…Ë:4\?4"P‰LEÜ?ïöNÖQœ?SºB?SbSïWǀ?SºB?ïÛh`^?p'@²1÷?rKÏÊÍ«?p'@²1÷?ïöäSYÌÙ?7pªh›R?R7Xд_"?7pªh›R?ïø†–~ÿ\?I"óæàRõ?Må¦sœFA?I"óæàRõ?ïÕfÁÕøÅ?tA·½Š?uLž÷vùl?tA·½Š?ïÖûÁÏ:2?{GSeá?t'B?{GSeá?ïâ.ÊTÐ?X­¨£,b?mÑ5£¹Ì?X­¨£,bAGN4FGL J0730.1+6852¿å*ÆR4U@<¢5¤À;ôrKvö×À=x,æ0@`ú'ùÄ'@6âÔv?Ö&DÉ^?íâþ1ɦ¨@u-fj˜$@~=F\…½¿ï÷Ìàméh?ì¦-['Ý•?ÏÝê@ûó¬¿äîÝ}I,¿ïe©!ÌÙb¿ðAGNbcuNVSS J072949+685305?î˧'Ý·Î?¥o9k(?£E‡Î´ç$?¥o9k(?éû°^k#?ĸS:‡?È>‡¶Su?ĸS:‡?ìˆ]vu²?£¼S"èßò?»½LW
m?£¼S"èßò?äOh{/î?±C¦i®ô?×a/ç	 #?±C¦i®ô?è$böÍÚÇ?ÍPHbz¥?Ïnt$Ȕâ?ÍPHbz¥?Þ/c¶Ö
?в\§(?àèuN$"ú?в\§(?äÃÇ>?½Z°
º?Öýòxqń?½Z°
º?Ë.^b6?²ÄëNd‰d?é4hgrú?²ÄëNd‰dMIXED4FGL J0730.3-1141¿jfMfQ@	ì:P]æÀ6ÂôÐ÷Ô¸À:ïø»h {@ÓÑ3¹ÀÖ@ ŽÉ[ÿ?ŒS¹Vç?·5Ed8@'€2¹¯æ@ç÷¤'Å:¿¾>Ž;Ô¿àñKÞ'ñ¿äÞDÄU/¿ä"BO/èü¿è=N	xNÆ¿ë÷ãœ*ÙAGNfsrq3FGL J0730.2-1141PKS 0727-11?ïé<~_¾?d©jþ>Êl?fÃøÆXr?d©jþ>Êl?Y<\?¶ò—üO`?¤_¤*l:;?¶ò—üO`?ïÊA-á~y?	í(¤?zßhï¤[s?	í(¤?ïÚ÷Âï©F?vÿR§µñ?r"—I¥?vÿR§µñ?ïÏ'–®
?vrùå'A??xl4Ž)‡d?vrùå'A??è÷LÓ Ú?Ðb>BIÀW?Ì"̱|—ß?Ðb>BIÀW?ïÎÓôÎ'?C¬'n¦Ø?x–¸–&û?C¬'n¦Ø?îrK""à? ó8³ÕÏ?¨ÞKEä? ó8³ÕÏAGN4FGL J0730.4+3308¿ëë0CÙbv@6NÆ6°–À:D¿Z'ÈÀ<mÆ	d-@æu27}?ýˆßØBKÕ?ÀA«›úœê?½T›bÇuu?ýƒ«kS51?ü8ÀA¤¿ï{œŽ@ ?ïñ¾>¶ì¿Ý!_€îýÏ¿Ô É°·¿ä´êÓ¿åÀ_–¾sAGNbll3FGL J0730.5+33071RXS J073026.0+330727?ïüvKÙ?Cµ¡º:°Ö??dMüyÍÓ?Cµ¡º:°Ö?ﵕÛôÝã?‡ñޫѽh?'šˆü™;K?‡ñޫѽh?ïìÐùµÁ¡?hÇ`°#³¶?c/Eß^?hÇ`°#³¶?ï9geü?~Cã¾X¦A?œ¼Íë։?~Cã¾X¦A?ïôìÂq»??L&Õi?V&{'ˆA?L&Õi?îÍÿîù•?­yaïÍó?£ °f²?­yaïÍó?ï䃲I
W?uYó°ù
?k|MÜpc?uYó°ù
?ëÍɚpâŸ?¨¡z~?XØ?ÀÈٖ<u…?¨¡z~?XØAGN4FGL J0730.5-0535¿é"¡]:÷@Xr)é–À9C_V§¬'À;û[Ð
nï@Oªú•@(šE'É?±ŸÑÛÄ?°ë	_
´@~%ŸÌ¹'@º'
ÛÑ"?ïîè¶7_¿ãDêJŒM¿ãI"â s¨¿à{ÿõï¿èiýà)¿ã,+6åo[AGNbll3FGL J0730.5-0537TXS 0728-054?ïýÁß2D?#S¶á‡Ýu?1öþøÜÖî?#S¶á‡Ýu?ïëuºŸ×)?läÈ–z"?dŠEsf¦ë?läÈ–z"?ïòMÖ°¯?QXú²)-¯?[eæ?`ÒL?QXú²)-¯?ïóˆ"Iß®?D âäã{?Xîׂ>#s?D âäã{?ïù¼¦RÔR?CAƒŒÐZ?I
gŠ‰™²?CAƒŒÐZ?ï9ߞðˆ?¦2Õ2Œ±?˜ÄA©Y?¦2Õ2Œ±?ïÙbz|%ž?{=Çí7?sN¦pQ(?{=Çí7?ïá¤âüî?ZƋþC÷?n[à&¡ún?ZƋþC÷AGN4FGL J0730.7-6602?ÚàtSŸÀ4ËݵR]À:(›)¼'ìÀ<Q7Âäì~@!>{ßI| ?û†×¥mã2?¸ûŽ^I·?§¯rÉÌf?ð$ύqm+@ó…'P¥¿ïäY`Äeö?ê$õî.Fd¿©7q@Ñƿޛ0þ$³"¿ÙXÜ¥‡äe¿Íóÿ*AGNbll3FGL J0730.5-6606PMN J0730-6602?ïþ÷ËËg?ê¹ô¨®X?.Ђ7¤x?ê¹ô¨®X?ïõ_¢ØÉ?TÐ'>ð%?U@¼U½?TÐ'>ð%?ïîé'ÞÈ?dˆ@
œ
*?am<´àI?dˆ@
œ
*?ïðh½œÐ?I&¬Á•ûÖ?_/5ot?I&¬Á•ûÖ?ïû(ƒ"9?<²'—D?C]òo÷Ué?<²'—D?ïØ»F<¥?túÂê¥ï¡?sþ¢X9`?túÂê¥ï¡?ïì+òQ—?rþãM×I4?cÔô¡V?rþãM×I4?ïÖ	ך0B?fœ¾õn6?tûUCöœ?fœ¾õn6AGN4FGL J0731.2-1403¿éÚþ>gwf@–ù%ñ+QÀ:*Ógñ€áÀ;ʎo™ëÏ@ûL¶çÞ @/<c]j?п$ÃÍÕ?׈'=Y@·kcü(Û?ø›{HË Ó?âñn!›±!¿éçÇßþù¿Ü$ýŠ·¿ÞŠ0]¿î1ВT*ú¿ïùžrAGNbcuPMN J0731-1402?ì}QbA?µ1xú»é?¼wìí÷?µ1xú»é?æ(zŒQ÷?Ȋ}I#Vê?Óׯ
ç\?Ȋ}I#Vê?êèŒCÎ>š?ªMRáÉ?Ä]ÎðÇ–?ªMRáÉ?ç}ßiæX?¥¡C¸	Èá?ÑA,3ÿP?¥¡C¸	Èá?çOYj»œ?Ã&u 3Ä?ÑÝaM*ˆÈ?Ã&u 3Ä?ÁRúȉ?È6ùã?ë¼+zMÞ?È6ùã?á6ö÷˜¨X?ºbÛ}¥ÙT?ݒίP?ºbÛ}¥ÙT?Ç¥Àí#7?¤'¥I1Q?êÄ·29?¤'¥I1QMIXED4FGL J0731.8-3009?äuÙy¿šÆÀ–4T›bÇÀ:nb
·'À<'‰±Å@ n·Ã¦3@ʸ¥Î[B?ÃÝ
Ý~ Å?ÉÞ
¼×?Î*ÚÊ"Ý@åàÄüI¿å˪Þe{…¿ä¡L`«¼\¿Ø^ìŸ{¿èZa_ìNÈ¿Éŕ 
;¨¿è,¾|¨AGNbcu3FGL J0731.8-3010NVSS J073151-301058?ïü©4:D?1c }ë­ò?:·ft+]•?1c }ë­ò?ïïáèùåE?jÓ>½À>n?`Úk?jÓ>½À>n?ïòY¹—?aRdÿ¡±?[MþF±Â?aRdÿ¡±?ïý©wn\»?Ÿ·ÙBß?2´F^2?Ÿ·ÙBß?ïù>$¨ÖÎ?A"Þh†t?Km¥6Ó?A"Þh†t?ïš+î×tØ?ž]?y§0½?‰uWá:?ž]?y§0½?ïêoâˆmD?tE"E·+:?e=ÙLˆ?tE"E·+:?ïôlž!?O^""?VÅ',5ÞI?O^""AGN4FGL J0731.9+2805¿ë:pÊ@4¦£ßm¹AÀ;3x‰|ìÀ<·v Í|@ M«¤?þ{Ê`áÂ?Ю†ü#»?¼'îY?ìH^sRÝó@`¨܅ý¿ÕIÈ`u¿ë!ªªcy¿×ÖRß¾¿Óòó¨é¿âÒ;66ó²¿ïÿä¼­šØAGNbllRGB J0731+280?ïþëì¤? ÇG	ì¼?/¡>)'¼Ë? ÇG	ì¼?ïò¤gkM?[ˆu¨¯©?Z·2 J?[ˆu¨¯©?ïñvÊ?P.ø?]ÁÿÅl¹?P.ø?ïô°,$™?8·€
ei@?WÈ é^L?8·€
ei@?ïþ¹SÇZ?p
^>ø?$jÒ'ŒEÀ?p
^>ø?ïÀ™§u>4?†¤–'?³,g
£?†¤–'?ïòÎWwœU?e<mõI?ZcPø
&@?e<mõI?ïќ…ºÈ?bIÇE?w1½BèFI?bIÇEAGN4FGL J0732.7-4638?·sr/]ÀÄÀ)«"«CIÀ9ù±ñ\ÏÀ;·×Ñã@"ñ>q)ä@Õí6´È?ğUÆ0%?ß±Þ¿"~M@9½ÆŸŒ"@oÆÚðQ?ÙÉÉã
€ò¿Þ—$'¯À¿çXàÚö±¿íÞ[€px¿ïûE@Pýô¿ðAGNbcu3FGL J0732.2-4638PKS 0731-465?ˆ#
Ø?°W°ÂµY¯?¦$—|ók~?°W°ÂµY¯?ï᜻j­Q?oëzå1ô?ncDÊì—'?oëzå1ô?꫅eÒª?¨X'[?ÅQêk̵X?¨X'[?ïÇÈ3¾|?dݟ®2º1?|æ2Ÿõ‰?dݟ®2º1?ï{F§{¦â?•°ð¦°SP?—+‹#Æ?•°ð¦°SP?ï@bôÊub?¬Mïê6©°?—ó¡^MÅ?¬Mïê6©°?êyéX?°6¼h™"?Çïö[Ò ?°6¼h™"?î	†ûB'2?™q-'IA?¯gIC'ã?™q-'IAAGN4FGL J0733.0+4915?琣ý(gÜ@:ÄÝ?á—_À;Ž"çƒ1xÀ<ÇÓØZ@ PÊwGà@¬Á¾¢h?ΐä>X€J?¦ƒÝ‰wQ?×ì$ÁUuR@ƒ,,®´´?ïÉ÷šÖ°{¿í',ˆG¿Ò–ñH­ü¿è]b
â¿×óµÄÈqs¿ß¤L%šAGNbcuTXS 0729+493?ïþƒ"°·Ô? Â)ŽÇŒG?'Æ´œŒ¸•? Â)ŽÇŒG?ïóÍNÑg?X]ª·myß?Xed,S0Ü?X]ª·myß?ïòteL$?Q'HWÒ6?[Ûlawö?Q'HWÒ6?ïù¶¯î´?1ªhP2n`?K±$Oz)4?1ªhP2n`?ïþ©õm'? täϛè•?%`¨§6ÿ? täϛè•?ïÈE)»÷N?e«
þ?{Ýk*Ci?e«
þ?ïò,[gÑ?fð»21?[§I‰ü™?fð»21?ïßɧ†õ±?a`enê‹?p,4ö¸?a`enê‹AGN4FGL J0733.1+5910?æëª)xŽ @<KªX-¾À:¾åžTê=À<¼:ìe‰@£³1fª@Ûä—Å?‰Å!Ý ?½Ý¨<I²Q?ö-íy¾Ô?þ:|PªC?ï¹Ö…³2È¿à˜›¢ˆU¤¿á½Aԋ³¿å^ˆM@û¿è܄›Ó¤¿é ÷IíAGNbcu3FGL J0733.3+5904GB6 J0733+5909?ïò¯¥Óq?Yác!­bÆ?Z ´œÏ\?Yác!­bÆ?ïÒX7­?v&½?¤MW?vÓä)pøÍ?v&½?¤MW?ïÅ®•?yhLCŸAò?}(ðq'Š?yhLCŸAò?ï1µ[äNÁ?xôTBÒÙp?™ÉTŒ
-Õ?xôTBÒÙp?ï‰ö¤j5±?‡Fqñ` ?'Vó1'?‡Fqñ` ?ï\
‹È?Ÿ¶õ73¥?œt~LÏ ?Ÿ¶õ73¥?ï")´ž?"Ρ•æ?œÏzÅü ?"Ρ•æ?ë²*0n÷s? ç¢w=I?Á7W>D"3? ç¢w=IAGN4FGL J0733.4+5152¿ìW%%Q/@;PÜY1ÊÀ:œ˜¬3ÐÀ<'·I­Èü@ ëË|Àšå?üWu¸e?¾Ú¡ Ì~H?¤õg £#?éUM9n·@)Òh@Ž¿ë"Š.B¿á՚ }#¿ß½<:¨¿Ô;»P¿ã1Vº ù¿¾™AGNbcu3FGL J0733.5+5153NVSS J073326+515355?ïþ¤·@.Õ?ÔX@׎Ä?%´‰ÌRlŸ?ÔX@׎Ä?ïõ}<¬Ò?T|'sWµ?U‡º-<Á?T|'sWµ?ïùJcrão?=º}õ"¢?JÖrœædR?=º}õ"¢?ïö·Bˆ!?9Àöà¡û2?R'{G³ð ?9Àöà¡û2?ïýàý (?&ªbÃHÌá?0øt´é¸?&ªbÃHÌá?ïÐo?d*2?~·Z¿P!Õ?wÈ`Hk†è?~·Z¿P!Õ?ïú¢P!€ƒ?\6	,yÞ?Ev¿˜Ç?'?\6	,yÞ?ïß`'?]撏œè?pOð«À·ç?]撏œèAGN4FGL J0733.5-5445¿îz¦Ç!±À0-VJQ]À9àª_ºz»À<M‹^¿@ô¢""EB@?A^o!?·ÐK\tË?±š}Å'¼Ý?ø–ùáØ͌@j¼¨'Zá?ïûbví'¿ãŒdý°šg¿âdøbQÙ¼¿â/! 8B¿ãɵÁŒä¿ì"~w=AGNbcuSUMSS J073334-544544?ïþÏÁsÓ6?Jz&Äï?#éBW±³?Jz&Äï?ïõVÊ£8?Z"ˆðÆÓl?URj=Ýòi?Z"ˆðÆÓl?ïõÕÖG3?N¶ã[€H]?TTRóƒú?N¶ã[€H]?ïþïäÐ,?
f®µ¹	?!þKþ?
f®µ¹	?ïþÞËZv?H­î8é?"G?b¡?H­î8é?ïÚSIÂÛv?~EòdvK?rÖ[4í?~EòdvK?ïð$sZsG?k掸<¹n?_·Ç(si?k掸<¹n?ïþ7Rãä?"¯Š'åu?,Ž›Î¥"?"¯Š'åuAGN4FGL J0733.6+3649?ïñ‡—©@7ѾãÕýÎÀ:·óáäŒÀ<'³!*3@x\fˆJ<@°Ò€jôk?ÂÇ·#Ã(´?¨÷ð€ÊÚs?ã:¿ïn¸@
<åc?ï´èâÄ0¿ç+zl­¨D¿áֈ7q†U¿äx#'¬?¿íë¥jˆ4?ÑUÛ}¿žAGNbcuGB6 J0733+3650?ïü*DÄw‹?6ÇÔh±y?>­ÙvzÏ?6ÇÔh±y?ïôs—§Q?Xëèjeæ?WЈ"‹·?Xëèjeæ?ïËv¿‹+ÿ?z_Œƒä­?zD J84†?z_Œƒä­?ïúŠnê€?15/Àz?Gå×F¸ ?15/Àz?ïù‡ôç¯7?DâÖÀð?Ià,ÅQ[4?DâÖÀð?ïÎa³Šl¼?€ÔûÅ?xÏ&]%¹½?€ÔûÅ?ïځ*âצ?}þAâ
?r¿jx–­?}þAâ
?ïëÀÇ·?RY‡ø໒?dæ?×\Ðí?RY‡ø໒AGN4FGL J0733.7+0205c¿äýÎnQ[+@$º±NÂóÀ:¬i—sN¬À<"/|@5@Í$¶n@è"C ç?ÑúeŒKÓ=?ϗ
Éĕ?÷›bÇuu@š1P/p?ޜJØw{?ïڍ¯ãˆ¿éÔ¿?E-¿äÙÇQbÉ#¿ëä¥Ï2¿ïÿú¡œGtAGNbcu4C +02.20?ïÆ|hRÇ?{,òa9áb?|Á˹ÏV?{,òa9áb?שׁ´Ÿ?Žß¹@d/?"ü>Îs I?Žß¹@d/?ïQ.R<§•?ˆ{»[bÁ?•Ú5½'wZ?ˆ{»[bÁ?ï†|¸Q.‹?q'~ØX2O?Ž`Ñë´]Y?q'~ØX2O?îóËdþîn?¤¿¸Ãÿ"? ÃI°?¤¿¸Ãÿ"?îbµ-c?¶u§¬¬ÆÈ?®¹Þ'nÔ?¶u§¬¬ÆÈ?렐½Á°Ô?¬Jaw9(ˆ?Á}½ù<±?¬Jaw9(ˆ?ì¤XXž…?¤yCzã|æ?ºÝ;;Ö?¤yCzã|æ AGN4FGL J0733.7+4110¿Çù2ÆѶ@9
»ìª¸¦À:=~|Ý¡0À<yy1DEª@i%u°[R?þÙ.T§!B?ÀêÄ.˜™¿?ª€câAm?î]eÖômü@ݤ]ÂÓпØC¯AÌ~¿å5f͔s¿áˌ%<Ðk¿Ö®êäâ¿ØãP÷,r¿éUÂ@þAGNbll3FGL J0733.8+4108GB6 J0733+4111?ïüØg=?0"m9ëÍ??¿H¶¢"»?0"m9ëÍ?ïô8B€qï?VEîþy7ç?WzÈ"b
?VEîþy7ç?ïõš\Üd?E|¦\½þU?TËG™Î?E|¦\½þU?ïîû€
ô?C'ùªŽ,?a€Gò¾?C'ùªŽ,?ïø!s\?A¨ûUåÜ8?Oz3ŒÇ;¥?A¨ûUåÜ8?ïÇlP¾¼ò?æ¿)Zž/?|I׳/jÅ?æ¿)Zž/?ïöÄðûË?dÖ¤ÿã¬?Rv †Š,?dÖ¤ÿã¬?ï¿8Â
ÉT?i\ÛWéó½?€1Ïrþ×	?i\ÛWéó½AGN4FGL J0733.8+0455?îÍh•."­@']—5;À9ÆØôù;ÁÀ<6	'_Á1@O}–®®@ÊZ¤'Da?º8vÿeÑ@?¾V§V›˜!@€ê[Sí@š˜jÅp¸?Å8(%
*¶¿å(Tf,Û¿äP‰OŸz"¿ä`
+Òì¡¿î`~oò¿ïÿâ~9ì¶AGNfsrqGB6 J0733+0456?ïô«ŠŠC?"ßú¬z?V©ø¼0ɪ?"ßú¬z?ïï%I"?f&¸f'l?`Úïx"ýˆ?f&¸f'l?ïÓ¾²ÇÎ?v÷øÎI*í?v ¦µ¬4Õ?v÷øÎI*í?ïýÀN~'?$o$F?1ý‹×ã'a?$o$F?ïõûyë?P€ØKëÄ¿?T	ï«·½?P€ØKëÄ¿?š1³Æ?ïM>òæ?‡Ùl³Öˆ?ïM>òæ?ï°±ùŒÉR?†	îQ)?ƒÓ­K˃?†	îQ)?ïú¬•¹?4Ÿb°·?EM©6‹Y?4Ÿb°·AGN4FGL J0734.0+5021¿ÕÙÒç¬@;$"ƒ‡ß]À9áj'"À<gœâ#v'@ðy©åE@&ÜB‹•Ë?·ëp&É?Ä¥"¹¾R@5\FR@Àx¿¯Wò?ïÑ>¶ôô3¿×þT.U}á¿ç6òl¬Ò¿çÆžEÑ¿èX.•>Á¿ãò,"à`AGNfsrq3FGL J0733.8+5021TXS 0730+504?ïû<¨Á™'?@æx³-´?C
\p¶Vµ?@æx³-´?ïóʉó֞?WžÛÜ4øÉ?XjìTËã?WžÛÜ4øÉ?ïÙªq5ÕØ?k8JÞiƒ?s*ÇSçá?k8JÞiƒ?ïòƒû:@?AYÖª2Ù"?ZùÁÏÒˆ?AYÖª2Ù"?ï÷É°b³Ô?J[›ª^¼³?PlŸ,Ùçb?J[›ª^¼³?ïÎCš^"?xLȜBÁž?xÞ2ºº>?xLȜBÁž?ïu‡k™¬?"s;=`?œÑOŒÊ~?"s;=`?ïËDxç?ez™½˜‰Ê?z|Ý©ovÅ?ez™½˜‰ÊAGN4FGL J0734.4-7711?ïØ\³À8
à"S.À9i)•ûhÀ;ç$¿ÒéG@=@ޗz†@nXæK#?²§òø°€f?¾³k§ÃÓÕ@
í$%y6M@žL[Î2¿áÓ_
+¸¿ßM"ÜIm¿ã¤;é»¿ä ˜%ü¿éã{dû,\¿ïïÏ0T[¢AGNbcu3FGL J0734.3-7709PKS 0736-770?ïüzTYôh?2'puRüH?<-_0¼ð?2'puRüH?ïö3§2š˜?TÔâ·op?S˜²þŸ?TÔâ·op?ïÝÀà…f\?ck<ò¢R?q¨¯*2?ck<ò¢R?ïþ´x9™÷?á‹/%>‰?$¸zá&kv?á‹/%>‰?ïööÐßà?QÝ^@+W?SÞþ1'?QÝ^@+W?ïÜ"¨v<?sìðïAó?q2M?sìðïAó?ï]Eö"V;?RŸÎÖ¬
?"WA2äԌ?RŸÎÖ¬
?ïü"Ð0üÅ?2•ŽþÏH?>é|'qº?2•ŽþÏHAGN4FGL J0737.3-8247?ïIqD¥–À9y¥CñÇXÀ9ڛ<1·À<8¸¤ Ü@ýäG'»¯?þ=þÈs¢?¶_l÷úøÚ?°ö!YìÛ`?ûz4ääÇ@9CiŒ5®¿ï£Ùqö½?ïÿxPsµÚ¿àý|Bם¿ÜS¿ð›^¿ÝĶv$J¿â°ÚÉÒ+AGNbcu3FGL J0737.8-8245SUMSS J073706-824836?ïüI0íÕþ?4ŠCaüsd?=¶x§M°?4ŠCaüsd?ïîÝtK²?`ÓTX Å?a"‹¯níœ?`ÓTX Å?ïâ]‹q?p!ß±Õr\?m¢c.-þ×?p!ß±Õr\?ïÔed€)¨?]?¿¼x«µ?uÍMºkËÔ?]?¿¼x«µ?ïðÀñ2˜ë?U#0âÆJ?^~QJÊ?U#0âÆJ?ï¾÷vøX?ˆœ'«¹®?€B"c©?ˆœ'«¹®?ïÂÀIå.÷?ƒ=Ý6·†?~ŸÛçä'?ƒ=Ý6·†?ï5®o†?‰Šä¯ssá?™J2!g
=?‰Šä¯ssáAGN4FGL J0738.1+1742?暣<ä›@2÷ß (À7@'§À:ÿ³"ý*c@[‡/‰°m?ÿ¬BÊ ?˜wñ†É?®îŸ&÷@Ý­àx{<@Õ r'B?É	¤C–­¬¿Ô<rwá¿á;ã:Í[h¿ßJål[¿âÔOb"Èõ¿ãY™~Á¦ÿAGNbll3FGL J0738.1+1741PKS 0735+17?ïö_ÙÀŒ^?X±ŒC¶‰M?S@L­¡ô?X±ŒC¶‰M?ïßOäCá×?p ˆ
ès?pX
ç­üc?p ˆ
ès?ï¬~ÿö?‰q•dBÚ!?"à@	>ôÜ?‰q•dBÚ!?ïÎ]lRõ¬?bD¬sæ'¤?xÑIÚ¤±½?bD¬sæ'¤?ïô<©dÎó?Z†ã™JôÛ?W†­ dšy?Z†ã™JôÛ?ïeÂkí0g?šXICöü?"G²Šðù?šXICöü?ï²N…¸Õä?‰iÃJêuY?ƒl^ èÎü?‰iÃJêuY?îÿ‹«;ÏÜ?Šfàt8é? ENÖ·8?Šfàt8éAGN4FGL J0738.4+1539¿íê2X—Ʊ@1O\žf‡ôÀ;mÄ@6PõÀ<½Üºí§@ °€¡¦‰?øT¨Ù ˜?Ø̙¡&V?âØ\î 0@t¤Ú¦@UîcöIž¿ïÄà\+¥?ٙiþX5?îŒÖ!à$˜¿Ò×ɓ\i¿æŽÏŒ0û¿ÖÃT¦Ë±AGNbcuNVSS J073824+153839?ïù7fžšŠ?Cè¤×€Óý?K"ejö½?Cè¤×€Óý?ïâb2¨t?q¸"«L?mÎû;?q¸"«L?ï³Oz^r?w:¿§Fì©?ƒ,!`í¿'?w:¿§Fì©?ï'P.Ê ?s® ø—°¨?‹~lçÎ?s® ø—°¨?ïíøÒì3?a¨ØÂGk?b-ç³ôµ?a¨ØÂGk?ïFí­Ëˆ?Ÿ›lݗØ÷?Œ.D'î?Ÿ›lݗØ÷?ï®5¶¬`,?†R¶R¯FÌ?"r'MXÑ
?†R¶R¯FÌ?ïy†Ý1ý?PWM+o?œðÏ2V\?PWM+oAGN4FGL J0739.2+0137¿ïE	Õ6º@&Á,I4&xÀ7')yv
£À;tcŠ	@¡œvmŀ@'>3Av?"[M¿·¡©?¸T=ë.H@ "¥Ξ@Wˆ"MÞ¿ÏòUk`K¿â³¼ÅîŒ:¿æL¢:Rf¿æ‰Ã}˜²¿ëÌ>1"÷¿æüÇ0«™vAGNfsrq3FGL J0739.4+0137PKS 0736+01?ïõK·Ïæ?Sd>õ}ã?UiôíՔr?Sd>õ}ã?ï·kSàý±?¡Ì
51;ì?'%+¡´?¡Ì
51;ì?ï´£èíA?…|ºqȝ¨?'×þLA¼?…|ºqȝ¨?ïýÏEš``?'s¾¶»£?1…Ó½5×?'s¾¶»£?ïä`ªî3W?bjɚŽÇ9?kŸUK†7?bjɚŽÇ9?î—òZÙs?·‹}'W)'?¦€ÚTü"ì?·‹}'W)'?ïªEU|<?‰ðÖ¾ÔkÇ?…n½.?‰ðÖ¾ÔkÇ?ïö€Gcú?J2a§2'H?Rÿq¥ۜ?J2a§2'HAGN4FGL J0739.7+1743?ãÃ×ìÌ®@2qWÿ›V2À:˜)W_À;mÓÐÍŽ@å4`t	@ôZDïô?ÊÀDÔt?²ëJç.ù?ï+üÞ@âaFkõ¿Û0³¼…à¿éË4çhY†¿éôàM/¿Ý´áÙú2¿èìЮÝ*¿ïùÏdVÁ®AGNbcuNVSS J073948+174304?ïûYåFÌ?@ëžé?B˜jÀ7¶g?@ëžé?ïñ-~µ´û?]¬¨9ümR?]¥úJzH?]¬¨9ümR?ïÂß(¢"?~)­k
57?~k¿4Ž?~)­k
57?ïò³¼/›¤?A>˜*ZÏ?Z˜‡ð§|?A>˜*ZÏ?ïò~ä¦L?b@rH3UÜ?[6ýŸRî?b@rH3UÜ?ï¼HÕ©6½?"ú#¢Áƒ?€íʝAt¸?"ú#¢Áƒ?îö ç'\?˜¯©"'? ñ†Ú>?˜¯©"'?ï~‹c~ˆ?›¢ŒÒm?/ΎhÅ?›¢ŒÒmAGN4FGL J0739.8-6722¿î!܋ܗ›À4nÑáÃôÀ:døÄ¢[àÀ<[~ùc@ñØSŸ@ޝ"ÐÜý?µx…ø§ñ÷¿µ€°®ˆ"?ÿÜazn['@_"ØaV¿äw6b'œO¿åHþaur¿â÷<b|¿ã9wÑ¿ßØB·4µ¿áWß_¡{:AGNbcu1RXS J073928.1-672147?ïþ¿ÑÅ7¶?æÁV"‹?$âUxsá?æÁV"‹?ïös«.¨›?XŒÂJܪã?Sª¢I?XŒÂJܪã?ïöcƬ€?[«¤"²¡Á?SÅ8© À?[«¤"²¡Á?ïþ…V–¤?†ÄßÞ?'ªšBaØ?†ÄßÞ?ïý=›ZÔ?2"Ó0?7Ö.¯R_?2"Ó0?ïÜ·m?t\qC±Ôþ?q¤u­ªn?t\qC±Ôþ?ïííÇvÕ'?sQª˜H¤r?b8H'1C?sQª˜H¤r?ïõIà–$¼?HÄþ9àþT?Ul>ñó÷?HÄþ9àþTAGN4FGL J0740.0-0753?êNÏ¿Ý@EàqÅ?:À:†_-À<ê°¢¦@µÏ‰?¯B@µj£	#?Ĕˆ7Çl'?¥ìã¼à?ß¿½WÓ|@P`ö:¿á
B[Ûs¿Ýbyýr-¿é±	ÝÏS¿é"ÛÈ¿í;'ô:Ïà?ã0} g(®AGNbcuPMN J0739-0747?ïü¹"MéÝ?7"A°Éýo?:3dÜ_5Ý?7"A°Éýo?ïêíß´u?s%»qÝ7?eè‹Û.?s%»qÝ7?ïڌ¤?pVûí%L¶?r¹­Ö%‡Â?pVûí%L¶?ïû-yF#6?-0´ÓæŠ)?CJ»pA?-0´ÓæŠ)?ïñxðà0?cëÀ*ñ{ô?]Ó@ßü?cëÀ*ñ{ô?ï56äÔ¼—?¦u¢6–Ø?™Y#^‰59?¦u¢6–Ø?&3ñI?†üÛù´Ž?ˆ6}R¦?†üÛù´Ž?ïÔlÀêã±?gƒ?©+?uɟ
‡³?gƒ?©+AGN4FGL J0740.4+7300¿èm*2X—Ç@=l" ٔ[À:¼³ÑSDKÀ<;&Ö-Ÿ@}EÐïœ@
«£|qk?"f7.¢¿Å±KgŸV@øpž2@×´³Pz¿³·†
¢¿í^ܙÉjB¿éͽ"¨™¿À'Á¦Ss¿ìû2Ál"¿ïÿí@_Á‡AGNbcuNVSS J074111+725822?ïúÚUD?N6Á󈵽?D–©™]?N6Á󈵽?ïÂṪ?'ËB¢Õ?~ó=Güž?'ËB¢Õ?ïw;³N)?gôÀb¯m?'GÞlÜ?gôÀb¯m?ïïGFëˆ?VwûD~'?`¸p¾"×î?VwûD~'?ï÷~8r?UNø­›š(?QüÜÏlA?UNø­›š(?î$¤¢ÈS?¶Ó¸žH~??­¾uºýÐ?¶Ó¸žH~??辰JK?‰›?³Š‹©?†½©ý€N?‰›?³Š‹©?퓷
©ãO?°I¢)mß?³bG©Ôþ‰?°I¢)mßAGN4FGL J0740.9+3203?磴¶¼¦@7Ϋ%(®À:®Ð!#~À<}æðdŠ@;Gxåo@¡ Ï?À<Ndçá¿ ž=ŠØ"?Þ®@dô÷8?÷úÚl1¿ªMìœöÆE¿å77¤±ü¿çÄóºw_³¿ØÒB­)¿ê0Bhv¿ìqýs]ÆAGNbllLEDA 1979979?ïó‡UA?YR&eR"?Xåðrãß"?YR&eR"?ïى™ÏÒï?€=§7ŠX{?s;2ù*"?€=§7ŠX{?ï¬IËÐÈ?†i*	?¤?"í;Ü1ì?†i*	?¤?ï®Ë™Y-?f'±®d]?"M9¥°V´?f'±®d]?ïÍ 6M¼C?sdÁƒj¨?yoäÕV—?sdÁƒj¨?ïJ'£ÄüÛ?¤Öy¥±¡?–¯«€,¬?¤Öy¥±¡?ï£±yú?†¯Ÿ5'
½?‡<ÿIR­˜?†¯Ÿ5'
½?í}hojB?Œ´Ô"‰"?´¼†2Óu?Œ´Ô"‰"AGN4FGL J0741.0+3226?Ùðoõíhµ@7òu¸eÀ;̉>؂ãÀ<çH㞠@#/p-ºxa?õ1©u¯¯†?ÙVùvy!?ÔÅ:çÝt?üGZ·ÜzÀ@œ0K¿ï÷û^ۂ?î3;5t¬¿ïÿÿ^ðP`?ïÿþó…õ¿ÔŸÕÖÀ¿ÛÒ݈óAGNbllNVSS J074054+322600?ïù_æÌR?kÑ.ÄvB?Jƒ¤±ÅöG?kÑ.ÄvB?ïó\¶H³?X;Ñèï…ó?YF'§µ*¸?X;Ñèï…ó?ïÄÃ@±öÞ?uöð…ŽGÊ?}ž_Š×Å[?uöð…ŽGÊ?ïùÛT5Gœ?AÑ,^~?H'¯X'Çb?AÑ,^~?ïî—I'?bàðã²ã\?a=ꛐ¦î?bàðã²ã\?ïÅW!à>?€ŽlÂ³?}T8oàÑ?€ŽlÂ³?ï¦ò臜?†؜‹QÝ?†Czn}?†؜‹QÝ?ïàìÔK"Ÿ?l!¼Fük†?o+¹ëÁS?l!¼Fük†AGN4FGL J0741.2-5140?쬋›¡~À+Ÿ™€o&)À:oèuŸ¿NÀ;âŒÅuÀv@\ZôÃ6@™çZÌË?ÎÐè:fƒB?ȶUýb–Î?÷—'Ôà˜@±»ÚN¾?à;ÅþÒX}¿ÌÛybí`¿æàÍûü¿ëȬ¬›ÔÝ¿ïÿ$=Çâ?ïû…|¬#	AGNbcuPMN J0740-5137?ïñÁ™
D?Vä#.Æûq?\|ÍswYE?Vä#.Æûq?ï縸‡Š?qñæ#˜[
?hëGoSíŒ?qñæ#˜[
?FYøç?"0£ÌÑfÿ?ŽY®sК'?"0£ÌÑfÿ?ï܈¦!?Y^¯VÒò?q»­
ì\?Y^¯VÒò?ïÏkG̝R?|óµ…ç˜?xJ\,ï&à?|óµ…ç˜?ïqœàÿg\?š%äzšN@?'Ìcàt?š%äzšN@?ìvEVÜ?ªÄss%wÅ?¼MÕOAŸ?ªÄss%wÅ?î~¬Ð¥?™Õ<F¨?®Øƪ¦?™Õ<F¨AGN4FGL J0741.4-4709¿ëü–r·q`À'zŒûüÀ:
O"'ÉœÀ;üýòÆ@	ýå¶@©EÄ/oY?Àw€bæÕ?¼íÜ
n?ø©¡Ñv@
Q©BO†?ëö@äv¸¿åð×~+©ý¿èF¬â¡ N¿ëä3¡<]¿é¾Îqèz¨?Ú/‰E
¦1AGNfsrqPMN J0741-4709?ïýÿ-Xd?N€š¡E<À?0"1åß?N€š¡E<À?ïóG3VÐ?[/ø!ç?Yq™7ðE?[/ø!ç?ïàêZ@,/?qÞ<,ŸNô?o¥ÕÑQ?qÞ<,ŸNô?ï÷4üê?8?@kq(Ø?QÕÄ2€?8?@kq(Ø?ïüo"È&J?8"—Úiäv?<ƒØ«ìò ?8"—Úiäv?ïÁŸùô¼ð?—ÇD&ê]S?0ét¼U?—ÇD&ê]S?ïÉçùŠ+N?~ڑšhj?{TWtù?~ڑšhj?ï¼)óš†?pRð.{{?€õ¸¼ê˜?pRð.{{AGN4FGL J0742.1+4902?ï`Ê¿›$Î@<0_¿ƒ8.À;7—Œy À<º%œq»@©†f‹û ?þ¼‡Tów\?Øj×DÁ?Øoâ+XÉ?ÿQßá|‡:@åµ{øI?æZà‹Ær@¿çÞÖÜH¿Ç&£"o8¿æóá^TI-¿ïûü€¿¿ïÿÅþ&ŒAGNfsrqGB6 J0742+4900?ïô=c&¯±?RX§êâ™?W…9†¥žO?RX§êâ™?ïî^G^
|?`x¶Æ‡?a¡¸ƒµóÀ?`x¶Æ‡?ï.´ª'l'?‰ǨT"?š)j·¢ÑÎ?‰ǨT"?ï®ât1ˆÂ?dÖTe&E?"GbømC‹?dÖTe&E?ïï$z€;?]ÇÎOt­Š?`ۅM
‹?]ÇÎOt­Š?ïÃ̚;ÄÁ?1Ïzó?~²ÚŽ{‹?1Ïzó?îª=;}b4?šZ|ÁÐ?¥\,E–'Ã?šZ|ÁÐ?ï	ç¶nLË?ƒøÎ
¢ì?žÃ	)Ÿ`®?ƒøÎ
¢ìAGN4FGL J0742.6+5443?îykòu™@=øe×Ë.À8tÇåÝ?À;òc`øh\@š{ú!n»@Ê=p£×
?Šˆ¦úw¢?µª@8M@iæ@;Yr@üþËÍsf¿Ã§Íyps¿á¶vÛ)¿åÔþõhø¿ä_bцoñ¿éE¸põ6¿èŸ^ÕxlùAGNfsrq3FGL J0742.6+5444GB6 J0742+5444?ïÝgguã?­%^»û'é?qLLWœ?­%^»û'é?ïðoe'T?m	I\¦<?_!4'â¥ç?m	I\¦<?ïáWjÂc	?tƒÚ¯RWU?n¨•H›·?tƒÚ¯RWU?ïÿĤ"õ>ñºñ£Ú'1>þ=—5ÖØÜ>ñºñ£Ú'1?ïù"@FÂ?@
ùCÝ1?Kvÿ±z?U?@
ùCÝ1?ïÊ-ýƒÝ?‡µm?zéNEE¢?‡µm?ïç‰ZB|ã?u(' ûŒw?hv¥Ú_Ôq?u(' ûŒw?ïÿ";X
?Üê<Õ¬$?÷yU2?Üê<Õ¬$AGN4FGL J0742.9-5242?¤ÒoùuÀ,,©¬6TÀ:ê&yçMÀ;Ó·?œÎ@ÙqÍͨÀ@yÏ.´H?Åkøa%3ì?ӉU^?±@=X «Ó@òÿf}¿ï¯šAµ,?ï֘ȹAÖ¿ë+:¯(w¿ç±_ÞâÎí¿êzÇw"?׆·¿ŸgºAGNbcuPMN J0742-5241?ïÔñ»-Ø?'¢9§è‰?u‡9=åóø?'¢9§è‰?ïçïlÚt?iv9;aµ:?hð"%Œ,?iv9;aµ:?î‹L˜p5?—?T'Ý8?§K6|lKÓ?—?T'Ý8?ïß\@¢?Y·•Lʏ?pQßæ@üs?Y·•Lʏ?ïSõ"OÖ?Ÿ)AY¡?•OuÞÿT?Ÿ)AY¡?ï[]Á¹?° Ì
S2?Ÿ"B´ÞÙ?° Ì
S2?ëpq¼¨3Þ?­"ºýY—?Â>9
_0Š?­"ºýY—?íºs€.¿?¢~Hìi1?²,cþZ£
?¢~Hìi1AGN4FGL J0743.0-5622?ÍÿÂ度ÒÀ/G™€o&)À:@NK½m´À<&¯söqâ@p|ЋU@w@GD?Äym>Ç»ì?Ãô¾""¥?úmlP‹3@"¿ÍŠâÈ?ïÍa¢‡Sò¿æ<|óp¥…¿ëDžj䥿åzÁҝÇ&¿çz4y"P¿ïÿþ½à ¿AGNfsrq3FGL J0742.6-5623PMN J0743-5619?ïüeò€Ä?7‰ž0]´?<Ðmô¿\—?7‰ž0]´?ïô=ÓäÝÔ?Yïú +ñV?W"WìÇ{?Yïú +ñV?ïÊ8
»ùI?yµo>û^?zãú‰F+Þ?yµo>û^?ïøhQM$¡?40¤²ÀÛY?N^»KB,?40¤²ÀÛY?ïý±P?:‹ʪŒ•?7Êtýò]?:‹ʪŒ•?ï×`yx£?yôÆ*çR?tpÏ¡—'§?yôÆ*çR?îþÍÒu&?–
X5Ô«Ç? "ÛAò£?–
X5Ô«Ç?ïÏ\C'r?fpČÚ	?xQ÷½êó[?fpČÚ	AGN4FGL J0743.1+1713¿Ç;$™<|ˆ@2÷4Ö¡aåÀ:tt "ôÀ<UXª¼Í@îˆv܀@öQo^?À4X6ÍÇt?2¹ˆà?Ò
þ Vâ@"µW¿ìa>‰R¥?î'úC'œý¿ä£< oK½¿à}á,U¿Þ»ÎÍ®¿åëÐ}ÜNËAGNbllTXS 0740+173?ïû·F†TÌ?3>žÌ Õ?A"äþ­˜	?3>žÌ Õ?ïñ*ojF?^cÇYÅ=?]«!vLI?^cÇYÅ=?ïò°Ñf?P%ä\]¾j?Zž\Æ_3?P%ä\]¾j?ïò"ŸéØ?AÓxûxã•?ZØÁ{v ?AÓxûxã•?ïñåä²?Q^n½lŸ?\46#	½Â?Q^n½lŸ?ïÅQSNe?UÄ·èT·?}WVJ†ÙE?UÄ·èT·?ïé–êg½T?qŠö¡?fiМD*?qŠö¡?ïÄ^"£Eó?mç|â7òÒ?}н—¯šq?mç|â7òÒAGN4FGL J0743.3-4912c¿°²F1|I´À(ÌxB0üøÀ:Lâ\
WÀ<	_¨Ý|@®Ê_	Oà@¸E܃#6?Ŗ^%Ð;?À}Ãû
?ùÃk$;?îDæҝ~?íÌ:5…óÊ¿å{¦3Ûϟ¿è!æڕl¿èe¼ÝÁf½¿ã¢©][û©¿Øˆ§ƒè‡AGNbcu1FGL J0742.1-4849cMRC 0741-490?ïøbË.ðŒ?OŠoål›?NtÒÆåªj?OŠoål›?íЬ–ÝË?³€àq6§q?±z›I…$?³€àq6§q?ﳌ=ªIY?ƒdÕ7—N?ƒð"]åÃ?ƒdÕ7—N?&  ?'ïí§ýy?¯¶vüº?'ïí§ýy?ïÆþ.n¨T?‡‰Y¹"%?|€è¼M=í?‡‰Y¹"%?à^EsZHT?ÑÁUáŪ?ßCuKoY?ÑÁUáŪ?î¸î…ш?ŸF
@ï¶?¤q¥{3¯?ŸF
@ï¶?Þ§›¹y"?¼"'Ã8?à¬2s£Co?¼"'Ã80MIXED4FGL J0743.6-3805?àÆzX"IVÀNÁ;ŸÀ:A¨@üI'À;Èu2²ô@Ó .^7@¥Q]À¥w?È-Ûõ‰¯?¸[&þWÅu?ñۑ¦†'@__ô²D
¿Ø"€}¾Ç¦¿åOì!%êu¿åUŸ~àÛ¢¿å›û©Y*>¿égõèO	S¿ïü<@øî"AGNbcu3FGL J0744.1-3804PMN J0743-3804?ïý ¸š?'j¢†Ûz«?3öù•ðÏ?'j¢†Ûz«?ï0Iä?iܲ¡>?`kX¸XĎ?iܲ¡>?ïèrºû®?^cE¢´
ü?gçP!?^cE¢´
ü?ïüò×ú? ÆÞ/vÓ?8iEŒ+š´? ÆÞ/vÓ?ïý_O¬÷¬?,æGw;?5nJëå?,æGw;?ï±hpîè?š…kå+hd?ƒ¥ãômú?š…kå+hd?ﳃ´nÌ?ƒ|Pòð#?ƒ:ߍ—?ƒ|Pòð#?ïïŒàߺ?R4s¢?`ìsýŸ?R4s¢AGN4FGL J0744.1+7434¿Ûç˜RFÊ@='MÓØÀ:¾ù¥À<zŒþ€£ÿ@ –€
§Mâ?ÿ ¥&••ÿ?°¾ØmiåÍ¿ ‡ìa×OL?ðÂ0â (@7ÛÜ_;û?ç"5vÚQñ?d*®Ì©î¿åRÀâ]Ø£¿ÝB€Æ¿×1šânõ¿Í]v¾"eAGNbll3FGL J0744.3+7434MS 0737.9+7441?ïû¶d€ˆ&?67AW"ç?A&m¼s¦"?67AW"ç?ïòڊrÆ?Y_yЍ	?ZJë1ûôW?Y_yЍ	?ïò2$ÈêÉ?b'­"TÂ?[›¶,1ï4?b'­"TÂ?ïÚîí¢Ê	?V®þ§³?rˆ‰>i/Œ?V®þ§³?ïôãF`â?Oº¬(lR?WÒ9ÈÛ¦?Oº¬(lR?ïÍïüâŒ?x£úû:À?yq^?x£úû:À?ïña'üã?q.®8?]=°y¬× ?q.®8?ïs0·‹z¦?{Ã20µº?'™é«M?{Ã20µºAGN4FGL J0744.2-6918?Åø[NŽÀ4ÇR"ÃÀ:'"Nü½À<E[sÄû@סçñÁ@œv"œ;?Ɨ–I­óï?°1,a¡Ÿf?æéHcF v@GÂWþÅ?ïû¬´('¿ÚZ[@B¿äü‹Rûпæå§#Å×æ¿éù>Dß-"¿ïóˆù8e¢AGNbcuPKS 0744-691?ïõh¼ç§?P!1]4á(?U.‡±s'¿?P!1]4á(?ïï€y?eýÞ·ƒ?`€%Ÿ¸Ì?eýÞ·ƒ?ïË·¾C®?r©Ñõ©ƒ}?z$tˆÐå?r©Ñõ©ƒ}?ïã-Å=¿Ý?PUíFuZ?lÒ:‡&Û¥?PUíFuZ?ïВY‰^8?tŸñéÎ?w¶Ó6oú?tŸñéÎ?ïÕ™¡"Ó?uA!Kc[?uq35lâl?uA!Kc[?ï_ƒœ	éì?ÿ»Û'˜?"Œ€zt?ÿ»Û'˜?ïhO§)œ~?{¹
•Nb?'ö#cv6?{¹
•NbAGN4FGL J0745.4-2447¿âá¡°"\ï¿Ã<
ÍHÏÀ9¼1ˆ8HFÀ;]H2ž¹@¡Ž_S͈@ä4 ½?Ê>{eÒ?֋I?2É@¿)Æ¢ç @û
3\ó¿Ý9ÐÜ&$¿Ù†ðI©—>¿ìè®?Cî¿ê³¸þ¿ð?ï÷$ß³Y^AGNbcuPMN J0745-2451?ïœËbXT?¬»+Y‡÷)?ˆúM1¸¿?¬»+Y‡÷)?ï¢ëSò™?"£?ß5}?‡E+;½§?"£?ß5}?íщCnØ?žRêÿ)ü?±sµç$‰D?žRêÿ)ü?ï̋üD?eãá߬?yºÐ
0?eãá߬?î!¥¯B"?¶ÊN$Gª[?­å§âx(Ý?¶ÊN$Gª[?éZælŸÕ7?ÌV!ªt³?ʔfM€«%?ÌV!ªt³?è±I"êq4?³¿H‹Ò4)?Í:ÙìV;1?³¿H‹Ò4)?ì(ˆŠRª?°!0÷¯é?¿Æ»»­j²?°!0÷¯éAGN4FGL J0746.0-0039?ïð7jFè@'©Çy¦µÀ:¾?A^o!À<4Ÿá²7@4,}·eÝ@ûÙ_'F—?ʵ'ž}¯?‰Ú5b"ÑÙ?»æ'ølŽ?û÷-Uù†¿?ïÎúnƇ8¿ì	XÙµé[¿ì½ªðÙòO¿Í~(¤äÑP¿ïÊÿ'¬˜$¿ïÿ9+
ËAGNfsrqPKS 0743-006?ïœ(*Ò¢¶?œuÒÄÎp?ˆõõA~—?œuÒÄÎp?ﶼï×`F?ÓS,U|?'PÄ>Tj?ÓS,U|?ï4®yqþ?"BÚË1$?™|ª-b$=?"BÚË1$?ïͨź'?dÚT$½u&?y+¹g0?dÚT$½u&?ïÁ™´,Ô?"O.#sò?3&'?"O.#sò?î"-ç™×­?´t¿ˆî0?¦Í!…†ž2?´t¿ˆî0?ï[0{Ñ?—'…4C?´8·Ö?—'…4C?îóP³æf? g&là¯×?®°Êóå²¥? g&là¯×AGN4FGL J0746.3-0225?KCùÝOìÀ@&a·À9þoï|$>À<-Ý­sk@ fJ%3?ü<`Ÿ±?¼àC÷ü{f?³Á# k…_?ù×ÜEԉ@	VcȧN8¿ï‰\:­Ñ?ïÿñBÍÛ¿ä!¥Õèտϗ¯I.G;¿Õw•ì¼¿ä¾pžM³gAGNbll3FGL J0746.4-02252MASS J07462703-0225492?ïÿ¦/»@?î'8±–Ü?«3¾è©û?î'8±–Ü?ïì;úýv?i=ódú½?cĦr	?i=ódú½?ïôLñgy?a–Ñ•ïÍü?Wf)Œã?a–Ñ•ïÍü?ïúŽ–Òj?-dÚd¿s¸?EÇÝÙ}$Å?-dÚd¿s¸?ïþŸâLՊ?2d±þeÜ?&ÜÒDâæ?2d±þeÜ?ïØÿyâ?–°Ó9Pî*?‰À(fµó?–°Ó9Pî*?ïꈦqC?r2"Ré"?ewY©ÄØ?r2"Ré"?ïïê'?QRæ	êN?`o×=	?QRæ	êNAGN4FGL J0746.4+2546?ï¤ïjrP@6ފar
À9ºøW•KÀ<Ëùh6J@ó¿qÅj-@ýJ¡!?À2?WÙ°¶?П%ʔä(@	ÌDÑ	@ã$—9#¿ÖSb}£š¿åX&grÕà¿ìÅî Úk¿ìziR©ñ¿íeŠžT~¿ïý@'cAGNfsrq3FGL J0746.4+2540B2 0743+25?ïâYݲ%?l+­x3Æi?m¦"ô‹ª†?l+­x3Æi?ïòúšª)¤?\`±qƒ!?Z
Ê'»¹µ?\`±qƒ!?ïWÄ/s?ŠÂñùúNÞ?•z#°Ôâ?ŠÂñùúNÞ?ïøR"Ð?9?‰*æ¹?Nµ´æ>5Ó?9?‰*æ¹?ïÍó­%+w?sfÒp*V?y)|ˆŒ5?sfÒp*V?ïÉ°È+ʬ?}Ò:ÀàK?{'›þ¸R"?}Ò:ÀàK?î´M鱤? ({Â?®"»#øšÀ? ({Â?ïÒExã?eôzet€?vÝvî"âÁ?eôzet€AGN4FGL J0746.5+2730¿Ögníz@7|.º'®›À:f…8¹"ñÀ<ZÛýÂ8@Wxð+̍@2³Ïà?È*2	h?Ï/՛'Ž9?øœ"ê-/ä@
»
±‰ÐN¿ä¿ôa¼2¡¿ÚPfíÖÞ¿ê
d1Xh¿ænd!¿ï­ÞA¿=¿ïã~õ©déAGNfsrqOI 272?ïðø¥£ø?Uï—zJ?^µ»¾P–?Uï—zJ?ïô_P¦X?['›%è?WA^qàÐ?['›%è?﷘?ïw?u²Ç&Àj0?'ð2¬Ìd?u²Ç&Àj0?ïö×¹K ÷?<åUš?RPqý"G?<åUš?ïá㬯˜V?l(zÊ6F?nS‹€ñ¿?l(zÊ6F?ïÓ\ìȞH?umzCHmB?vQ‰€ãèb?umzCHmB?îíÁ¼£^ê?–}Îßaÿî?¡#ä99­W?–}Îßaÿî?ïÙRˆ§È ?c§]üü;?sV»²úçÞ?c§]üü;AGN4FGL J0746.5-0710?ì¤ÍÿŸ)s@! c¾ì9zÀ9ùÓ'é|À;úPA`ó`@µ¤ÝD"/@»;ªÐú?½_ÎÇ£Ã?ÊÛ¨‡É¤@V4êK@ÑâgÞª?¬MI£¦Ò¿â#BzMú¿Üt»(_šš¿àó 
Ì✿éÕùœ8°K¿ïÿÊ ¢¢WAGNbcu3FGL J0746.6-0706PMN J0746-0709?ï)‰˜3Ñ?˜/Š®°‡;?šÎÌôh[Ú?˜/Š®°‡;?ï"u~Ãe¬?ŒŽo~nï?‹" `T ä?ŒŽo~nï?ï9¡e¯¡?3Ãû¾9?˜ËÓM{{$?3Ãû¾9?ïlŸóGWO?jALØùu?'lš"²?jALØùu?èp›I®0?À'¢²k?Î='ÙG?Á?À'¢²k?ìæªYä?¸ó—íÁà?¸Ê¯Tø¿?¸ó—íÁà?ä‹ïÙ'ŠD?ºâäaûü?Öè M°ëx?ºâäaûü?ëè¤{—G|?œGZH¥ê?À]n¢â?œGZH¥êAGN4FGL J0746.6-4754¿ê€ù`dÕÔÀ&œYyÀ9¾Ó-À;줾Éç@i*»ëS?ÿØIё?«Ý`\¥â?°ºž¡ì#@"8T~Ý@Ö2ÊÁ?íÐH¢†'L¿à‡·ïÅö¿àÂ_
§y¿Ýe¯¼ñv¿àUó‡K¹<¿ä®mє²ªAGNbll3FGL J0746.6-4756PMN J0746-4755?ïþ¼k€¬Ž?'¸+?$9KГ«¡?'¸+?ïõnÌ2ë\?X
©K"Y8?U"h‡?X
©K"Y8?ï÷ ´fµ¨?@ËvqZ?Q¾–è] À?@ËvqZ?ïú±ÔpQ™?0×ÔE'Ø—?E8­ZÐ?0×ÔE'Ø—?ïþCt@f?"ÛÑ,
3l?+ȸAè.?"ÛÑ,
3l?ïÉh/OŠ?–ñ¸L̲?{KèYšÎì?–ñ¸L̲?ïón›$o\?aژóÓ?Y"ÊX×?aژóÓ?ïõ3…uæ?E§EoÕ?U˜õ¢^…6?E§EoÕAGN4FGL J0747.2+4529¿æRr0>À@<hpdìé£À;8F:vôSÀ<½Hɝm@–•-NB?ü±'<ÓÅå?ÖÅi–œ?ÒAIvk—(?ýËûf=K»@O_™m¤É?îi* :8?ïÑÞïäÿÉ¿é¬ðžŽ ¿Ã`–‡f¿æ»E»Ëó‰¿ïù!bü$AGNbcuNVSS J074654+453231?ïøQÚWÐ?FÔá^¿¶?N¸–O,–?FÔá^¿¶?ïàFJÖ׬?rÞ?sWð?o¹´ðλæ?rÞ?sWð?ï̬Éw,Ý?tn–ܹ_?y©›E}h?tn–ܹ_?ï ËÀÄg	?l&^ÿ4?‡Íܤ­µ?l&^ÿ4?ïêXßrÊV?iéö¢û?e§ l9j¬?iéö¢û?°H¡s?")†Gh…Œ?ŒXSñG?*?")†Gh…Œ?ïŠîÝÃÀ?ŠŒÖ9H{8?xEt?ŠŒÖ9H{8?îšTÁ¯?•Ws7ªó?¦Z³ìk2?•Ws7ªóAGN4FGL J0747.3-3310¿ïüóIýêÀôÎf*…À8–·$¦À;J®ö"0¬@¦iÿÎÿ@"œî¸°?©cðüh,?zFäÚ¤j?ч-@´8"«ËË¿»ëXÔŸg¿Þ¡MÃqð¿æ¡wI¹L¿áÆy³JE¿åsUb2$?¿ç2¡<ü
AGNbll3FGL J0747.2-3311PKS 0745-330?ïþ—©Ä"ô?·úŒ
+?&…cûcZù?·úŒ
+?ïòA 0Í?j	{²™ý?[Û}՛åé?j	{²™ý?ï㒧j›2?xI !ü?lmXgN!?xI !ü?ïÿ©äâ»?ßsâ,h,?
ê?ßsâ,h,?ïüÃS7›´?63PÒSV{?9ådL¨P|?63PÒSV{?ï¢ÈËq"(?œºKa•?‡MÍL"?œºKa•?ïÍ\2l?€ÍnʙYî?yQæÅÐèé?€ÍnʙYî?ïþlú]Õ?"œŒæ幆?)>ÀÊI(Ð?"œŒæ幆AGN4FGL J0747.5+0905¿ë&$	–ú@0zÝð,À:|]Îè0À<€ß©HcF@§e3‹rº@
Òä>š?½ëû€]—?¡ôsb€Ü<?æÃx?ô‡—5秿ï±×~¶ß?ïÿ´‰	)¿ân—²8Í¿âL^G³ó¸¿Üü³Ú¸rοÞüR@¿ÊAGNbll3FGL J0747.4+0904RX J0747.3+0905?ïøҋlt?Gy¸Ì¼f
?LµÑf0šC?Gy¸Ì¼f
?ïÄuOYÑÐ?ˆ^9q:Ö?}ÅX@‰4(?ˆ^9q:Ö?ïÞcþ?p۝@1dL?pýÀT­M?p۝@1dL?ï‹=Úߓ?rÙ0ßüy?>ð—‹B?rÙ0ßüy?ïïßÐñ.?Xn‡(ý?` 0©ù‰?Xn‡(ý?î™®Ÿ1«?µ7̹ïô?¦ney0M?µ7̹ïô?ïÓâ;…"z?|Vôo/c?vâ,ð¢å?|Vôo/c?í_*úClU?¡ÿI†@?µ¨/œkT?¡ÿI†@AGN4FGL J0747.5-4927?ݵ¡`ý	ÅÀ'ÑÀ¨ÒÁÀ:®rn²À< Ô¿ª¥@`Í p@ÍüŸù/+?ºšÒSÊW}?¦è©C¨Ù?ï˜ûC؜å@0Ûê÷Û¿àæäÀßXÁ¿ãQL=Æ4,¿æՒn,-…¿Þ¥€B/¥_¿ãì ¾üÕ¿éÙRKý."AGNbll3FGL J0747.5-49272MASS J07472476-4926332?ïüÈ>·d ?*6ºuµûV?9¾èÞtç?*6ºuµûV?ïñ¯cõÊ?a
º\k"?\¡7ÙoL[?a
º\k"?ïø&§V(?B9ˆJ?Oeb˜ßwr?B9ˆJ?ïó¥3šj?>$yºCSh?XµÌlb?>$yºCSh?ïødJ'Z8?B^ƕOíl?NnÕ GWw?B^ƕOíl?ïÌ´fØë?¿¼Ràr?y¥Ì¢lfZ?¿¼Ràr?ïïX®Óù£?l
WßÊ\X?`§Pî-eV?l
WßÊ\X?ï½¥¼q"?mÁ©Xµr?€–˜…äÛ2?mÁ©XµrAGN4FGL J0748.0-1638¿Ã±zùg×Í@Ù½¥è\À9cÆOJÀ;´tÇR9‰@Ê·ÚwZU@LԁÌô:?¶iqž'óº?ÃnœÊPœ@xq¡šð@f'ÞdNß¿ÇûĜ|¢é¿å#—ŸC|¬¿é–ˆ¢ÑPÀ¿æŒ¹6£*¿îT6ž!¾—¿ïÚ¼i¨:AGNbcu3FGL J0748.0-1639TXS 0745-165?ïÙ="Á:?¨PvML¶?sa|O~Ó?¨PvML¶?ïÊ8ßUÌ¡?ŒŸh½89?zão6·'?ŒŸh½89?ï¿ažo[?uh0²Ñ¬6?€'˜a"'?uh0²Ñ¬6?ïÔXð¨2?X<‰ø¦r?uӇĊ?X<‰ø¦r?ï‡ɝ ?'àÅÍá?Ž8œ'–Ü?'àÅÍá?î<6~þI?³55–åµ&?¬>¼•|fs?³55–åµ&?îŽ@qNÇ?›ž­h1Ë?§øìÖъ?›ž­h1Ë?î—}õp§T?þzÉé¦I?¦ˆ ©Ñq¹?þzÉé¦IAGN4FGL J0748.3+8511¿êžGœ@<5‹¤
âÀ:´úȈšÀ<"çä€G¹@ ¶–*´Š?ø+®9cÎÜ?ÀOJ*›Š
?Ç
¸À¦@	ßøØK@ó÷ƒ¯¢p¿ïÿñ¢o+1?ïþ©ôZ°P?Î\u éY ¿ÐÐFŸ ¿à†é~3a¬¿×š¤ÆôE¸AGNbcu3FGL J0746.9+8511NVSS J074715+851208?ïò³î¦Þž?X'i}MWÕ?Z˜"œED%?X'i}MWÕ?ïâé_2H/?mó\¤8?m ¶ZxÔ?mó\¤8?ïÙlÁ'Ú?q*¦P¶?sIŸˆª^½?q*¦P¶?ï·ÿ±Y1}?dIñp7?'°'Ø«?dIñp7?ïè+Ä:=O?d‹©Ì A?gÔ<»0Ó?d‹©Ì A?ï`D€Yùé?¨KG¨Àf?"÷oôÀÂä?¨KG¨Àf?ïŠó¼®O<?Œ_Ru?C×ÛÍ?Œ_Ru?ï
Äít&?‰Ÿô[ïÛi?ž½§eÁ:?‰Ÿô[ïÛiAGN4FGL J0748.3+4928?ìóGT@=AÿÅGÀ:µbÙéëÂÀ<Žn‰J—@€§i»Ûc@ü&V«Þ?ɝµÝòå?ÀçàúVGà?ö懈õÝg@²ê%MA|?ën0Ê£&á¿åÑ£€ùÊ¿ä¨ßá¿à–Fދ¼¿ï¼F¢{Àk¿ïZü¥Øl=AGNbll3FGL J0748.8+4929NVSS J074837+493040?ï̓ŒßC?§$òžËÂ?yv>GNÎ8?§$òžËÂ?ïôu<k?TBmEs?W‡´¾Zé?TBmEs?ïۍ)ž´á?stè±$e?r9k/õ£G?stè±$e?ïÞ'cç¨?S!"êþ$?pð6ފKµ?S!"êþ$?ï÷²@Úe½?O‹Ë¡úXã?P›~Mô6Â?O‹Ë¡úXã?ïÉæì'@ã?~BîÀ|,?{‰­ºz?~BîÀ|,?ïÓ;j©?'&qMÞý?vbJšOnu?'&qMÞý?EŽ¸?sǑk'?.£;	ë?sǑk'AGN4FGL J0748.6+2400¿Ð'·Ôî@6»³"ý*cÀ9T²ü(À<+%üéË
@ñ~Ý֊@S·RDÌ?²J¬azŠ?¯JŠ¹'B?÷ëýáAÏ@³a+"?áÓ¦¥ñ–±¿ä& !]ž¿ãÏâÌ'ª¿ã©&4G/i¿å'«_ê¡I¿ïÿþR€ÖTAGNfsrq3FGL J0748.3+2401OI 275?ïþay?'d1XËz?)èj†$*?'d1XËz?ï÷2ýOÄ?Tæ°16\÷?Qý™Ÿ¬Ù?Tæ°16\÷?ïòËæ•B?aÕ©öÏ Ú?[Ôh}
?aÕ©öÏ Ú?ïþӌsó?3û€Ø?"Ç;dªí?3û€Ø?ïþ­~?fسjj?%.ñiaS1?fسjj?ï×´Ðß?va:»éSÚ?t|¥º[¨j?va:»éSÚ?ïÝ×{sá?zz³Š'ù?qBSÍâ•?zz³Š'ù?ïþ䡙‡? يue?.Q¸Kî˜:? يueAGN4FGL J0749.0-3904¿ç¨/¾«ï)À†?¼À:€ø¿™ÞcÀ;üFñ'@ 
=Šzò@+}\L1?È	<¿¤?²¯«~É^®?ícQÞïå?û½Ö½f}c¿ï`À¹n ?ïãÖ3}Ûοçxâ>ùæ¿ßøelkc%¿á}h@[9â¿ç
¢µ¢
ÜAGNbcuNVSS J074915-390336?ïüܦŸ?2Ñ«•ž<y??AMcæi?2Ñ«•ž<y?ïÔ	Z©?€ ;ggËÊ?uû@cÙt?€ ;ggËÊ?ïë…Läë?XX–&@?dz³Bi´]?XX–&@?ïżͦ;"?biPÓð?}!™>À.(?biPÓð?ï÷$
È·â?I]VŽúså?Q·ä']?I]VŽúså?îÜ*–è y?±Íá1Ï)?¢=VŽâCr?±Íá1Ï)?ïʺÐdË ?~a"voL?z¢—î–oœ?~a"voL?îÛ"B?ƒèMú?®WâLaë?ƒèMúAGN4FGL J0749.0-2956?æݍ.ÁÿÀ[íœP-?À:…ôÍzÀ;ނ€x`d@!$ÎÏÜKÆ@ŒÝÉtS?ÌÚväãÅ¿v«ÛKÑËË?ªŽ' cµ?øǟñøUg?؝¯]¦#k?Åíxé˶!¿Ü¤·$D
¿æ
š"U•^¿À7œ¨M¿ê¾;Ú¡¡¦AGNbcuNVSS J074913-295658?ïøH»?o¦&´6‹?Oãªd%?o¦&´6‹?ïÚËÁÆ»?{jb4(­?rš!–=?{jb4(­?ïÆr­Çxû?|,oþuPa?|Æ©9 :d?|,oþuPa?ïâ#D8û/?VûkY^þ?mÜ»ÔÃ@{?VûkY^þ?ïí?Öþ?aýà`Àn¡?bÀùî
º?aýà`Àn¡?ï¥Åæ˜j?¯K|WÎÏÛ?kGJ*À?¯K|WÎÏÛ?ïrÌÒÅÎñ?ñюßsœ?'¦e¬m‹é?ñюßsœ?ï:´Žèe°?&ïþ·?˜©n?&ïþ·AGN4FGL J0749.2+2314¿ì‰Ùö´…a@6–Κ,fÀ;˜+ÛPÀ<ÖÖ@ ÚêYûsÿ?ÿJ¹t*t?Ä#ÛýA^Å¿"=Ý8ÞKƒ?ÑÚ@þ¢Ý»?úñ¡µòÀ§?í8"ñœî?ÕHÒ¡ø㬿æq®ÞÐ/ƒ¿Üå<hš¿àO×äXÍ¿Ðq‡+ØÌAGNbllRX J0749.2+2313?ïýŸ1LíÞ?(%¸ÒäF
?3s÷Ú
j?(%¸ÒäF
?ïê:õ…ŽÜ?j¸‡ '¾?eÅ
YtäL?j¸‡ '¾?ïñ‹wÖH?aaÐ/"òd?\é÷Jà,?aaÐ/"òd?ïÓa(?WhÆT¼Ò?vOwjz\9?WhÆT¼Ò?ïü˜•É¼ˆ?/E¼ngv~?;;Rc!6'?/E¼ngv~?諭Ÿã_¶?–™"ñQ,?…PX(n?–™"ñQ,?ïõg–oÌ?`"ªôÄ8X?U0Ò·ó£Þ?`"ªôÄ8X?ï šŒ*<·?†µAx—ר?›ì®uÿ+?†µAx—רAGN4FGL J0749.3+4453¿Œ>åï!O@<¨1zÌNùÀ9ݍƒá¡pÀ<sn]«¬Â@"'Êö@o¡—Zû?µºµ|Ô?À0µS^w@c<æ:\@
щ5ô-º?ïèB©È»Æ¿Ý꣢\
î¿ãÔÖáΑž¿ä†J!aN¤¿è ÈÝ~ö«¿ï÷½ ‡_AGNbcu3FGL J0749.0+4459SDSS J074916.88+445232.1?ïü)X°?<\¡IâHº?>³ôwâ·?<\¡IâHº?ïòÅÍT10?_ÃiÑ?ZteÈPÐ?_ÃiÑ?ïåçsþ:¿?e mÈ­EÚ?j‹Ék©$?e mÈ­EÚ?ïÝÁ¢Tܯ?V5»¬F£?q.¸Ä?V5»¬F£?ïßÞþ¹À?kœn«g?p€—qKŸ?kœn«g?ï'nÒô|?ŽŠ–eÀ?}x»$D2(?ŽŠ–eÀ?ï3çsA@<?"Q8øM"?™ƒ'°Ž?"Q8øM"?ï'í9?s²ýEx?‹""oÌý°?s²ýExAGN4FGL J0749.4+1058¿á%¶¥ew @1Î=ÁçÀ:*GÒ&©À<J.oL@Xž¸ge@ø¨ê'?¸?W?JÂ?wâ?Âç?ÃÓ8KËÛ@¤©Ü‡ÕÍ¿Ñt
~^)׿ç¼Ä¬lÚõ¿çi'"š\¿Û/[ßyοæÀÒ@Ìú¿åâ,EhAGNbcu3FGL J0749.4+1059TXS 0746+110?ïü;Ï'ß²?/õùIÑÊ?>!ˆp¢°?/õùIÑÊ?ïñ2£W?`¥¯ááZ?]š¹=!ô?`¥¯ááZ?ïôõ¶XŸ²?Z¤ž<æð?V"u<;ö?Z¤ž<æð?ïõ±qkkù?>—¾ËXpN?Tižò?>—¾ËXpN?ïõ¾m¹kò?LOdrŸO[?Tƒ$w*œG?LOdrŸO[?ïÆØ#šD?ƒÅ˜&£?|"î"ÑØ?ƒÅ˜&£?ïçÉý±éi?u6:€*Æ÷?h6×E?u6:€*Æ÷?ïԎÙæÕ{?c@l™À·¿?u¸"Cî??c@l™À·¿AGN4FGL J0749.6+1324?ïŽkbF«@2ÝËݹ"À:űg¸ÏÀ<uTZË'±@·‹òçê?ÿb¡e?õ¹?Ð@gä•ÁH?àsNÁ¯r@v&}BJþ@Sò•í=¿â·îÿQ¯J¿Ý§!ïi¿Òo,Åǿ敏~¤™¿ïûæàõ"׿ãJ½É#ÊàAGNbcu3FGL J0749.5+1320SDSS J074935.95+132156.0?ìn4Ü´)?·™ì¨CÝN?¼ŽY^·,?·™ì¨CÝN?íÀŸÆö?±Þ
Ä$6à?±ûÏ1,Ó?±Þ
Ä$6à?êA»í茂?¬cz«pE]?ÆùH]Íø?¬cz«pE]?íÕ
ûeš?QC¶ÛkC?±W—ç¶ß°?QC¶ÛkC?äN'$/_>?Æ+++t?×bÛ·¡A"?Æ+++t?à…þÉ8›?ϸ¦5o‰·?ÞômòÉ?ϸ¦5o‰·?Ï*düóŸä?¹šŸ9Qìm?è5fÀÃ?¹šŸ9Qìm?ãQUތpo?´p8ë6¢Ý?Ù]TBç"?´p8ë6¢ÝMIXED4FGL J0749.7+7450¿¹öΗÁìä@=éSXl¨ À:ð‹+AÍÀ<³ çTº@ )'_
ž@N~:˜'B?½ÿ ‡	7¿®"ä¼é¼?ïñà'Œ7@ël‡è—.¿á!‡Ջ¿ì·¬ª–¿Íõ:ꌦA¿ä¬©áæ9…¿ÐîqãD"¿ê݃¬8XAGNbllRX J0749.4+7451?ïýƒaÚ÷™?(Ø È?3äòL»ˆ?(Ø È?ïô¾E s(?WGÿŒ'l1?VƒuÏ`X?WGÿŒ'l1?ïòêáH/?dDÀ'§¸?Z+ÐBï?dDÀ'§¸?ïùÎL¡Ò?1ºŽ>¼]r?HÆÌíêrl?1ºŽ>¼]r?ïúž¾—?@ÓÃgT#à?E…¼¡`w"?@ÓÃgT#à?ïÒµîJ18?w]zú³#?v¥هŒ!?w]zú³#?ï÷0Qg·Û?guûQ;ÿ,?QŸ]ÅX¼?guûQ;ÿ,?ïÜcÄÄ?b¾£/?Á¶?qÎx΁¦?b¾£/?Á¶AGN4FGL J0749.9+1823?ѝÌæV@4ëßÁœ"À:eËΠ¤À<ÑEØQe@w–÷Cï@ÀXeã‹?ÂáðöLÍä?¯5z`Cb?êæEy†Ô›@	7>$þ½
?ïýU–4ŠK¿èž¿=˜¿ß×µž‡êð¿ì0¯?ž%š¿Î?|í'hs¿ïÿÞ˜–dAGNfsrqTXS 0747+185?ïýüېèy?+Μ% Q?0"WOY?+Μ% Q?ïóÈ
­±?[Æx|Âä?Xoäoš?[Æx|Âä?ïÝ[hË4?s
ŠB"ÂM?q~Ò1}]ô?s
ŠB"ÂM?ïý_-jF? ÂÐC9KD?5ìÓwq? ÂÐC9KD?ïýÍ¢NÆ?6Ü,š—±?1'î,%_?6Ü,š—±?ïӘ+c
Ê?xÞñm?v3êBƒ?xÞñm?ï¼£1¦t?'R!…Ó\?€ø—;}}?'R!…Ó\?ï󉧴?Mÿ·
»ÁG?X찏£Ð@?Mÿ·
»ÁGAGN4FGL J0750.8+1229?åŽÀžQuz@2¼… ¾Q	À9g¥‡À<E8ï4×@à–ºìûk@äǕU?°Â5o"¢—?³K—ƒñ$@"ºkáÐ@.Ó8¡²?î¡À_@˜¿âDÞ¥gX¿èŸJrÉK¿ãÂð	è·¿ëÌùÆ·à¿Ü¨ÿéåAGNfsrq3FGL J0750.6+1232OI 280?ïýg·tK?&lÕ'¦˜t?4ÂF`:Eà?&lÕ'¦˜t?ïóœkŸÐ?XߺOóŽ}?XÇ)6'ˆ¸?XߺOóŽ}?ïæb¬êђ?löö&Buû?iSCéÄ?löö&Buû?ïý¢gQ•?"máƒIÜ?2ï4ç‰g?"máƒIÜ?ïýiŒ­ð5?) ¤ú½Åo?4³›&ï?) ¤ú½Åo?ïÈàœÀô?¸	+Úǵ?{±«4©Ü?¸	+Úǵ?ï×xË 'à?x…
ðRhÑ?tCš…#ç?x…
ðRhÑ?ïú"O$T?8ˆeÿ3V?GvÈWá>?8ˆeÿ3VAGN4FGL J0751.0+7908¿ïÜÅW¯á§@=gT~–À:ŽàùÀ<ƒØž'&ß@n"ˆ7Ç?ÿŽÑõ*¹è?¹.fDØw%?ÊOʘ•Â@ m֝0'@t—>u†•?ÈA•Ì…0¿Ê³!€nÅ¿á	}±Ç¿âÌËN¿ëB‰Œ¿çŽd²1@AGNbcu3FGL J0748.5+7910JVAS J0750+7909?﵈€»®?¬5Ï®ø%?'ßûXön?¬5Ï®ø%?ïópµD1?Y#Ý'¹C?Y–3¬¬{?Y#Ý'¹C?î_^ç/éA?ž†Übþß?ª
ˆµèý?ž†Übþß?ïøÜìïEâ?2$1&£?LŒMR|Èu?2$1&£?ï<t?"Çšñ£êØ?˜b)Ò#ˆ?"Çšñ£êØ?ïÇó^(v¹?€›%TŠ0D?|P͈¡?€›%TŠ0D?çhRMÄrÐ?²÷›Œ]Òá?Ñ/[dw`?²÷›Œ]Òá?ïëÄ*"#¨?Q=|Cˆn?d;ÕîZx^?Q=|CˆnAGN4FGL J0751.0-5131?ßå,·e~×À(Ç\¢˜FÀ9‹B¾ÁqÀ;µgôÛߏ@ÅûI{@mÆâ¨e?®Ðó"!?ÄrlN'@Dä]ã
&@ØP¹€ë¿Ò7¡¢&°ï¿ÝÌÔ#Ù#¿æ§¾ aŸ¿å`Âl »¿é™QÀg
Ö¿ðAGNbcuPMN J0751-5134?ïé"žÄƒ?bOŽzÚü5?fÝa[˜ä´?bOŽzÚü5?ïóK2%?cþä":Ip?Yi›6i(ý?cþä":Ip?ï°2ÊzŸ?}L¼a̘?ƒóMa[?}L¼a̘?ïÿˆè,µÒ>ÿ&g€¥çø?
ÅûKº¤Œ>ÿ&g€¥çø?ïÏ¢¥0üw?unŸJ&¢~?x.­u@4S?unŸJ&¢~?ïÈiÁ˜Câ?‡%\ÆU«?{Ë1ãT?‡%\ÆU«?î!"'@+?¡âñn›'ß?­î··äI?¡âñn›'ß?ïþu—9u ? ý-KOÔ?(¦bËÒ8? ý-KOÔAGN4FGL J0751.4-0421¿æáÛ4Í×@&¨?NÊhÀ:v6¾/À<k;÷'@k•\É¿?ü5g‹)"N?ÐKÚ®?ÑjÇôö·'@£øôõ
?ôr!èÝúr¿ã™µž2µ¿á1†:A¿Ôy_ã•f¿Ùýh
«T­¿ãí˜>¥­#¿ïÿêњ'çAGNbcuPMN J0751-0421?ïëÏ!nmO?dÁðE¢t?d0Þ{•1‰?dÁðE¢t?îýÛ싕0?¡DYÊlb? "A8""û?¡DYÊlb?:œ!ù?ˆ¦…ƒÚb?ßq\gÁ?ˆ¦…ƒÚb?·"p)?'i沫Ö4?¦'äŠ(™n?'i沫Ö4?ïÞVèD!˜?nØ$4¸Òn?pԋãn"ø?nØ$4¸Òn?ç|#°šxM?ʸ¼R3Ý?ѸžËf?ʸ¼R3Ý?îÂÕI6]?š·Æ²ÒË?£Ò®ÜH(?š·Æ²ÒË?è™fËæó¿?®¬ýYʆ'?͚dÐd1?®¬ýYʆ'AGN4FGL J0751.4+2655?ã\TD®c^@8Tòù‡@À;fØ9¦ëÀ<ÍcЉð¯@; Ákš®?þ'¨¸]ª?ÔÙÄ❙ƒ?ہ¬]@¢Ý@Õ™Qu>@¾ù:!E¿ÕêÔà«"?Î9íwYo?¦dƒ7W…¿àÏûÀÖ…¿æ¨Zý|˜¿ïûC½Äò
AGNbcuMG2 J075139+2657?ïüXFÊ?:0qŒAÎZ?==Ðã°}Õ?:0qŒAÎZ?ïðªIë?_û¿´?^«kçüFl?_û¿´?ï¯ô+'Ý?z"†´›|?"õ!°vü?z"†´›|?ïÒÞ26S?U1;é4Á?væÞÄ
¤?U1;é4Á?ïüà}{"X?34²uE•?8ü&3 ¹?34²uE•?ïÇÑTW+?0"Wøo×?|v`#>9?0"Wøo×?ï¦y n¹¶?…vø9J?†a—òv?…vø9J?ïr¼ŽŽ?xÖy:%Û$?'¼èåü9?xÖy:%Û$AGN4FGL J0752.2+3313?ÕÝ]Y³‹Ä@:lʁ˜ñÔÀ8÷tü+_)À<O²ÅºŠ@ùãÏrÄn@xô›Gïƒ?§-€Ä$v?¾}p@é@ˆIDíoÛ@ |ò–?¬9¥=;ʱ¿â?"À´W¿æFñ¡B…a¿æ"ύd¿ì@9
ãˆÑ¿å›«–òAGNfsrqOI 380?ïòç;–Œ§?WF#~I?Z1ˆÕ¦a?WF#~I?ïô]TïÆ?\æî?WÙE¨— ?\æî?ï¦yý¨?":†hÙ@?†}ᘐùñ?":†hÙ@?ïÿâ^Â>ã½Äôúf>í¡§Ãx>ã½Äôúf?ïö¬ØÛ×?P2AY¡«S?R§«½°À?P2AY¡«S?ïËí>1¶?Ýˉ>P?z	sÈÙàø?Ýˉ>P?ïÍÞ/JÆM?'þz{ꄵ?yèmÚ©z?'þz{ꄵ?ïÿЀò"ï>ó/JÚ¼À>÷¿ƒþ¤€p>ó/JÚ¼ÀAGN4FGL J0752.3-1631¿áÜ©†*@«Oag#%À9ÕVÅßrÂÀ< szK@ #@vè•?þ&ƒøG¥?¼ºD^ÿ"Ë?Á̈ĵ&=@ucߣi&?ú"®LˆÅ?ï…þ|rAf?äl{‰
Z\¿Ú,̼±¡£¿Õ»m߁…Q¿æÎ[}Õ¿×*Šbo
ûAGNbcu3FGL J0752.6-1629NVSS J075223-163340?ïõ'îË>?Q2ªÎ%Œ‰?U°!ûJ4?Q2ªÎ%Œ‰?í)‰nÝ?³«õ]Äê?³ô³F•›?³«õ]Äê?ïÄ&Á=€?|[1šzì»?}ìŸwí]ú?|[1šzì»?ìr'mš& ?Gæã=@?¼kl".Îþ?Gæã=@?ïkn8ò¶?‰µÀÙ³ìÕ?''8þÙwF?‰µÀÙ³ìÕ?âc´$+ж?Ò<¿÷¯×ý?Û8—·¨^•?Ò<¿÷¯×ý?îhF@^Èk?¡eÏEV?©{›úï`P?¡eÏEV?ã3útê|z?¶¤2ûÈ?٘+?¶¤2ûÈAGN4FGL J0753.0+5353?å˜T&%j@>8Go*ZÀ9
Ó	ý¯ÄÀ<:wÓv4:@åø˃K¤@±Èd?¥*.B؏?©× –V!@ÕY;¸Ì@o¥åW]4?í¿ÂWþė¿Ü³_=}9¿â¶2÷¤ì¿ß‡¼Aº4š¿æ¸¸
"'r¿â}i[
AGNbll3FGL J0753.1+53534C +54.15?ïúò)Úf?6=£ÇÿôÙ?D7§+í&?6=£ÇÿôÙ?ïèQ²&è?lìUܼ•?g®MµßX<?lìUܼ•?ïðÏêÇÆ?féØe /?^aþPìZ?féØe /?ï
7×:l–?Š$Xðt+R?žY'¥5?Š$Xðt+R?ïë×T˜¼-?\hk]ÍäÅ?d(«G§k?\hk]ÍäÅ?ï´ÜÉ¢©k?ƒ¢›Q{Üé?'È͙
s)?ƒ¢›Q{Üé?ï̐·´?å¨Ÿ²?yû·¡
‰î?å¨Ÿ²?ìð ·ê?¨å05Æ?¸~ÿþ5?¨å05ÆAGN4FGL J0753.9+0923¿áTyîՆ@2g,®À:Õ±°ç"À<ZzyBáý@½sO­è0@¶¾`"‡?ÈïèÛ¡&?Ô¼K?™s@>¼ž_ç@h	S»¿?ïýCÂÍoŠ¿â'‰¢€õ¿âzSƒ4Ó¿åùP¹Uø¿ïÿþÐñ?í–Ö;
˜	AGNbcuTXS 0751+095?ïÔÀ™°,?ƒË"Ã1º+?uŸ³,eæ?ƒË"Ã1º+?ïíMÀQ?eñ]üc¬
?b²ñ$2æ?eñ]üc¬
?î¥g‹³­?–µóÂZ*?¥©‡I8&?–µóÂZ*?ïìÒÒ±yp?Kã•c×{?c--9èç²?Kã•c×{?ïßQÜ¡?vdoM1?pW{sµ¯?vdoM1?ïœoðö?Ž\埆·w?ˆúäM¡?Ž\埆·w?íg–"M÷§?¤Ý˜tºï?´ÃK]"OH?¤Ý˜tºï?ïKáB®.?…‡ÜŽÓñC?–ƒ×¥Ս?…‡ÜŽÓñCAGN4FGL J0754.0+0451¿àáöj*R@0$ã—­À:|­""aTÀ<~Ç¡é@ÔÈÜÓ*4?ü(æÞÆÊT?Ææ¾ûÓËo?Ç­œZêo@Wþßn@RbÊÐs?ïà&±D±
¿ÑiòâáH¿Õ'-ks¡¿Ñ´Î¾¿mê¿áarŒÖ¿æêB^IasAGNbcuGB6 J0754+0452?ïüIÿdà?0c¾XW8?=°Þ+]?0c¾XW8?ïêÙP¤ïI?hˆ-O]O*?e&¯ŸÈæA?hˆ-O]O*?ïè67ÁÛ?nbÁd½…Ž?güɲ@¥|?nbÁd½…Ž?ïÛÞÈV5?N9¥ÈuŠ?r›ÞQÂ?N9¥ÈuŠ?ïø݅gï?CL>šE¨Ë?L‰êò}ñZ?CL>šE¨Ë?ï–öÐÉ?'óÁ'i?ŠB{'¬ò:?'óÁ'i?ïËI‰Z:?€zbý'EÊ?z[}ÆQ¢þ?€zbý'EÊ?-/?rOE=nñà?Œô°ià\?rOE=nñàAGN4FGL J0754.4-1148¿ÀôÂÓ,jö@ w9°$öZÀ8À"Ú›§À;­c¤G@êìž#l@?¶~¬®I?¥â‡ÁwP'?¶×ÉU"@ÅÐãe–@	û?ˆ??ãÕ6":¿×æÎÁ¹Š¿ãR­·]Ï¿¿á¡'bD˜¶¿àkö"o³í¿ìGÊϜŠæAGNbll3FGL J0754.4-1148TXS 0752-116?ïú'"Ÿ¼?@´õ¶qéŸ?E»vó¦Ú?@´õ¶qéŸ?ïœóÂô¡?• Gnå¢?ˆý"gî?• Gnå¢?ïÓëю—L?€b5±h?v
Iâf?€b5±h?ïŽõ{9(¸?k­Bêõz–?ŒB¡#÷b?k­Bêõz–?ïëŽÿë:Õ?`'U6;›û?dpÿÐûÅ?`'U6;›û?íђY^k?» zÚøŵ?·¡slY%¨?» zÚøŵ?ïUÅr¡™T?"Mæ6#)?•GQ¤í˜?"Mæ6#)?í_­¶~?š@C£) œ?µ"¦3?š@C£) œAGN4FGL J0754.7+4823?㩔¥'ʺ@>%–À8þáv§ý
À;æêð¤Bj@ào
¤É£?ÿ¸lrïá¥?§Ÿ!Ìa ?¶	8ãÌB¹@Ûwb7,½@P°ò{³¿áM¶ígw¿Ý;$-ܲ¿áQ"'›¿ßbÓ^â8š¿ç—'¾
è¿ç½w>û¾RAGNbll3FGL J0754.8+4824GB1 0751+485?ïý
‡RR?-6+§?7"Àm¯£?-6+§?ïòžGu¬Í?XN4€
2?ZÃq¦fm?XN4€
2?ïä)ê£ç?oGñíˆR?kýÖOˆœ?oGñíˆR?ïõ"6D?>¯–²½½?UÜÙPè÷?>¯–²½½?ïþ!Gg6Š?$&8þÊå»?-ë†Þ?$&8þÊå»?ïő†>ŒÇ?…­©â`3§?}7<Â}v?…­©â`3§?ïÛKó•Ü?·:b~/?rsÚ$?·:b~/?ïÚòP®²õ?_ÏñÀÝ5g?r†×Ä#eH?_ÏñÀÝ5gAGN4FGL J0756.3-6431?æüً]QüÀ1¼¡œZÀ:֞©£ÒØÀ< ö¼Š@ Š›QT±]@´¨+-?Çù¸¢ž?;1%ß/?»hø=¾Ò@€?Œ‡ã9?ï•[¬£7¿æe"®£¿Ìw3=D.-¿ãE=¼h|¿àgAøÈÔ¿ÓK‡½ÏAGNbll3FGL J0756.3-6433SUMSS J075625-643031?ïý@T{NÍ?+	á9Ù¸¦?5ý[hkä?+	á9Ù¸¦?ïô{ðfYü?Z¤¤¼Gü?Wò?Z¤¤¼Gü?ïòג<qå?ZÛ'ˆ¤µ?ZPÛ!gÆp?ZÛ'ˆ¤µ?ïõ†ƒ"šñ?9€—(ñ,?Tòù™ÍÞ¨?9€—(ñ,?ïû†6nÇ?7ø¦<8Ä-?Aç&=~ßå?7ø¦<8Ä-?ïÝY>'O?sOù|(%«?qStÎ^ta?sOù|(%«?ï÷Êßë@?aw»Yz<?QÌjïoã?aw»Yz<?ïݬýé>6?\"EÜBŠŽ?q)€î",ø?\"EÜBŠŽAGN4FGL J0757.1-3729¿ÑJU÷áÖþÀß}úâ~À:­"àòôÀ< F.¸z/@"æìސ?ûV¯TÊ?Íá c6?ȄiF?ªe?ü¯©öÞï@ìIŸSÃ?âSˆ¾*´¿ïÆ~ŸBP?ïÿú÷''ý¿ÙiÉ<Ÿm™¿×c(ƒ×»h¿Û`~oòAGNbllNVSS J075714-372734?ïýÝ	:e?&Fӄ0Má?1¹xó ?&Fӄ0Má?ïìe
BU2?q+`ìOA?cšò Î¦?q+`ìOA?ïîÀ—à1?`QxÍ*'?a?hUhå	?`QxÍ*'?ïél'6·?RïSÝê*Ò?f"õdpè?RïSÝê*Ò?ïüX훾&?@
]
Ïë?=8'ÚgF,?@
]
Ïë?ïl >ú;Æ?¤åhIè±?'kø¹H?¤åhIè±?ïȿþŸý?€RN³—?{ "Ùl?€RN³—?ïÄZ‰
…?rè›ÀQr›?}ðÒªK1p?rè›ÀQr›AGN4FGL J0757.1+0956¿åÅ&³#Q@3Ø{V¸À8¾Ø»™À;ëùŒHx@
Òw[¬#@ý¶ÿÛíÒ?¤™,v«®?£Ï@ ?þçp6ÉÀ©@"®%lÌ¿ÄÙn[Ra!¿ß$ÑÜFw¿ã<æÀ"Ùf¿â¥ôñ¯e¿åC5ªøh¿Öß³#®ZòAGNbll3FGL J0757.0+0956PKS 0754+100?ïþ6;Ñ<s?|ÀÔ#"˜?,œDrµ?|ÀÔ#"˜?ïðdƒ&)y?]ª0?_6ùòåÝ4?]ª0?ïó/MW?e5&|½R?Y÷¡Ù¤a¢?e5&|½R?ïåRØȌ)?Zjçãã?j­'sìö¶?Zjçãã?ïü †?8¢Ão ì??Ë
Eªž?8¢Ão ì?ï¿b—
.?…Uì±ô£8?€?gZ=tf?…Uì±ô£8?ïê-æ?B?vH⪬&ê?eÒí$¿}³?vH⪬&ê?ïªkÈk?{ÛG7ñ¹¹?…e:£­@?{ÛG7ñ¹¹AGN4FGL J0758.1+1134¿êë¸ö+@@3ú\å´$_À:ŸÒ¡"$À<}၏·™@ˆßµ\Ã¥@úz¡'¶?Àñ'êRï'?¥B#ªÃÒ?å†Å&6@#¹˜'‰?›v«Ô¿äQ›2öÍQ¿ç7"+#¿ÜWGd˜…ó¿æ¨î#;n¿âLÜõ)AGNfsrq3FGL J0758.1+1130TXS 0755+117?ïþ%ùþx?àâ-"/?- aÃW?àâ-"/?ïó†ƒx?Xç@d'«?Yøò–>1?Xç@d'«?ïùÕ^õ6?SRY.¾†?Hªƒ€, <?SRY.¾†?ï÷ÓØsÛ?1ûކçى?PXO+Nþ—?1ûކçى?ïûaƒ0T9?<D7" Eá?ByònS˜×?<D7" Eá?ïÏÌÜðŽü?}Ê%á7©??x'¥E%¤?}Ê%á7©??ïú³åA°?Wôxoá:?E0k0Æa?Wôxoá:?ïÛ5¯©P?\AX]¹Âx?re(E'à?\AX]¹ÂxAGN4FGL J0758.7+3746?ì?¡3Òüx@<áµ ÝDÀ;+"7ÉÀ<³bØ<l˜@\lû+@èy=Ùc?ÏBH¤ßrí?´~<Pé'?å÷SSd+#?ýœ"Áéð¿ï,æ}wúã?ï¬{­¿ÑPÜÚ¿Ö!yÍKwο꫇½Ï¿ÅoU®2XAGNrdg3FGL J0758.7+3747NGC 2484?ïøÌ>©ÖJ?BAâj]¥<?LÏ#à?BAâj]¥<?ïê¾Af9?fXR¦èõ?eA¾žN‡?fXR¦èõ?ï½æ"ìX%?v+<¦ÇÓ?€†ZɹjÅ?v+<¦ÇÓ?ïÊI_øì™?^ùƱ$Á?zÛPèKs?^ùƱ$Á?ïó4ô*D?U¦Ç)Ÿ¶"?Y–Â1ñ?U¦Ç)Ÿ¶"?ï›ãÅP›h?™" 0YQ?‰½1ø?™" 0YQ?'í–?i_Á\Œ?¶*ã´?i_Á\Œ?îùWVÏ?Š×¤kP? oʍ3X?Š×¤kPAGN4FGL J0758.9+2703?ìÚépœ@9ðr° ĜÀ9òÛª¶"À<mžƒä%¯@R­²«8}@Òáüߺ?¶'›}>o?ª°CÃèçN?ñï
D& ~@yıJe¿Ýpä+Ž#¿àJ¾ëÔ¿ãÑ.[]¿Ýó‹=
w}¿å'6É?¿è7fhê¥%AGNbll3FGL J0758.9+2705SDSS J075846.99+270515.5?ïü1X$.?E`⊛¿z?>wãÁV»ò?E`⊛¿z?ïô4|Qñ?V_5"·a¾?W—õYÒ¼ø?V_5"·a¾?ïñ0)ç?h¹P®??]Ÿ®|`è?h¹P®??ïߛã(?UÌÒú—r?p2{¡º¼?UÌÒú—r?ï÷wL¦™?Gö/B÷ð?Qå<.!?Gö/B÷ð?ïÑÊ-hÌ{?xÏnJ‡ùä?wéGz: ?xÏnJ‡ùä?ïá\ÚݗÜ?|ö®RMQ°?n£$çNÛì?|ö®RMQ°?ï(ÎD4ý?x÷€ä›½b?µÌd£ìÏ?x÷€ä›½bAGN4FGL J0759.6+1321?âü-["¡@5dàTiÀ:l¸ÿÀ<eä«æ£8@!K€0¼á?ú™C¬Äð?Åޒ\ŽvP?»«w¯?÷)sçXiN@®¡úçr?ï'h@Žf¿î˜›Ø8:Ú?ä^C¯'9¿ÝʢԀ˿Ãn9ÙënN¿äyT¼AGNbllSDSS J075936.13+132117.8?ïþüÄمº?C÷CK? 3°tv¸í?C÷CK?ïóÎðØ3¢?[U³Ží?XbÑ' ?[U³Ží?ïùUfdæ?SƒË{dâo?Jªh›6'?SƒË{dâo?ï÷°e/|?;BÖLN¯?PŸ5>µ?;BÖLN¯?ïþþ "of?¯­gãþ«? øÀëŸû?¯­gãþ«?ïÐ4"ZD?Hñ¡š%?wå¶q¤Y§?Hñ¡š%?ïü¼õFò
?Ayr¶7Έ?:Wi&°??Ayr¶7Έ?ïðÄC™æN?RúÖk@?^wy$)c$?RúÖk@AGN4FGL J0800.3+5611¿É?'țå¤@?³df±æÀ;:V=#wÀ<ÐÍ;‡•‹@ ­%èqï?þJå†×õö?Çy €"?Áþ"ÅõB?øÛkEÉ7í@;‹Œ:¶_?ï¬)¿*å¿Ø±ÁQ™{¿çýÀTïEž?î"ó—'Ø¿å€ê«Ú便åŒXž&ÇAGNbcu1RXS J080017.3+561116?ïý¿B—÷z?'2¿
	?2ì"Äù?'2¿
	?ïï¼}
5·?^Þ*ie?`C'·±ñ?^Þ*ie?ïô¼‰¢op?\§ü&5W¨?V†ìµ¡À5?\§ü&5W¨?ïÚ*~ój?QnÑä>?røê§/4?QnÑä>?ïùÌþ²b?FZd"Åz?HÌ2~?FZd"Åz?ïǪvÞ?y꧘¨µn?|*¿ ª?y꧘¨µn?ïðgÀXZ?l©Vðæ~B?_0>A‹¾?l©Vðæ~B?ïfLwtM&?}§¬á°Ã²?"6q¾:?}§¬á°Ã²AGN4FGL J0800.4-2257¿ç–ÿ¾ð@
戢ÑPÀÀ:L1ž½dÀ<S±Wü@@*°,Øü@…/‡­?ōi(dM?ÙÁZ]™Ž1@w¡øì@`[ÁqÏÑ?æŽMÀÓm?ÀÂQÔÒ*¿äé¾4ù‡¿åîoês¦Á¿ïÿñ7n+¿Ù¼®;è
›AGNbcuPMN J0800-2302?íÒÌÒ<_?±Àãéi¨ ?³i—¶O?±Àãéi¨ ?=½'?©gL€¼Fû?¦&l,LYã?©gL€¼Fû?ë#P¹?
?ª%¸ñ)¡°?Ãr¿Î?ª%¸ñ)¡°?îø¤_¬t#?}pöH*k? uº8½Ð?}pöH*k?é®vËì۔?Âè¿HÍÈ?ÉF$ÐL'²?Âè¿HÍÈ?ãØLµÍ?ÑoÛcØ0r?ØOgû֔f?ÑoÛcØ0r?á§Ë#æuQ?¹åZ.º?Ü°i¸3_?¹åZ.º?çŠ_RÝá?©½ƒK®½?ÐëAZEú>?©½ƒK®½AGN4FGL J0800.9+4401?ï"צ֪,@>‰ˆÁÛCÀ:Y:ßÏÞÐÀ<ŸOœ†@'ä¦èb@\ºÞ¿q?ÀuF©Éô?ÁGwÖø@1œZ>:@
åÜæuje¿ë¾«Â0O¿À*lD̹¿â¼,5èð¿â$!È`¿åeˆ…ug¿êœÞ|w AGNbll3FGL J0800.9+4401B3 0757+441?ïþ¥Ð'1Ï?7`xÈ?%¢ôŒ{n?7`xÈ?ïöVò2Àz?Röì÷‹?SR>»?Röì÷‹?ïðXÜKV&?p-ýjT¬²?_NGž¹?p-ýjT¬²?ïú)"§äz?-†µ Â?G[tæb_¶?-†µ Â?ïûàÆ W±?=í*…4?@|èP¢õ"?=í*…4?ïНˆ«N'?|öŸ¬Gº?w±;¾ö_?|öŸ¬Gº?ïïí5‰¶?jq»få?`ÊÈ9¹æ?jq»få?ïíO
Ú3=?PêzÀº®?b°òUçJú?PêzÀº®AGN4FGL J0801.1+1335?äeˆžÅ[@5yj&åGÀ;UDêÜ0À<˜'6ôˆÓ@GCeÛQ@oå]½Jy?Ï_×@™"P?®3‰ð.PË?â{wN:@M€VQ›S?êم!½j?à-‰Àނ¿ì\Þþ'¹¿¾_g¥«¡¿év±'n"ÿïÿûbâMhAGNbllNVSS J080115+133643?ïö~Ñ0"¡?OC€0¶Ä?S^íL©?OC€0¶Ä?ïåÀžÁ Ç?mcn"3Ä?j?a-@ù?mcn"3Ä?ï¿È±zç?yo|»˜—?€
Ó¿'J?yo|»˜—?ïÑ!‡F?[-ì•öË?woxžÐLÍ?[-ì•öË?ïØh/z}0?rôR\l?sËè`Nã?rôR\l?ï™MÉ·n—?ž{hº±?‰¬‡Õ†a?ž{hº±?ïy)zÞԝ?‰öµ	Ò?ÚЛŽf`?‰öµ	Ò?îû'xú#?ZµEV'R? FØt©RÓ?ZµEV'RAGN4FGL J0801.1+6444?ç¼K@¬SÂ@?¿#FV%§À:ܯæ8óÀ<ͼª R@ïÛ›l@^	Zõ?ÀQמ?Ž_^E–ÉA?Ð(€ý–nA@±ýx¼)g?Òdè'4ù¿å|, oa7¿ä& Z¾h¿Ú•ï ·E&¿á?›÷Aë]¿àLÜ¢,æAGNbllRX J0801.0+6444?ïÿ5 ïJ?
á¤w}Ip?\÷°ü¶?
á¤w}Ip?ïö"ö¶;?U².Óâq£?Sÿºҙ?U².Óâq£?ïû‹3؛?,îz݀…§?AÓ3^E?,îz݀…§?ïþf¿@‹û?к‡rÆ?)"¹­µÈ?к‡rÆ?ïþúò؂Á?n/ ÷`? PÔÝZ÷ð?n/ ÷`?ï×Ò0RÇè?z[‹=ùœL?tçê‰Çý?z[‹=ùœL?ïý4"¨,?T}{áa×#?7\Jåñ?T}{áa×#?ïüv£þÕç?)'ñÒ"#'?<Jàçj¹Ô?)'ñÒ"#'AGN4FGL J0801.3+6631?Ê3XK_hµ@?¥yžQ?À:Ö§"þÀ<£dύqm@î8­Ež@©¸ËŽ?Ë{«r	1Ø?ɔçÙ³Ñ?öl×[œ@¨»R¦ëè?é'ôÛߏG¿â̎\X¿é¦Ê;"¿âa‹¶'¿é–lˆ¿Vÿïþí{˜ý'AGNbcuGB6 J0801+6639?ïæâ-˜OÔ?®ŠM;" ?iÒ¨HÓí?®ŠM;" ?ïï"'I`?\ô¤Ç;
«?`Ý÷¡r?\ô¤Ç;
«?ï±
0ÀS?±|…þ?ƒ¼³Ùò‰O?±|…þ?ï͟ª¢!ö?Z`½èRï?y0*£ðE/?Z`½èRï?ï¶2">ûW?ˆ…»Ð¬ÿs?'s[8(D&?ˆ…»Ð¬ÿs?ï¾ï¤	¬t?€ª"}Jåt?€DþDÏ?€ª"}Jåt?î‹Ø(®Ç?œaQ\F°q?§B}t¯‹?œaQ\F°q?îçyØmK?†|4yœ] ?¡ˆbzù[?†|4yœ] AGN4FGL J0802.0+1006¿ÖXÈ×Rjd@491"·ºíÀ:€®@ð‹À<zÛmy€@Ÿ*Þzõ?ÿM"þ1ɧ?Á#ÖÉÐÃý?¼)m↝?üI¬|]?ûÌpk¢æI¿î1ºÂß
A?ÖW•}«&Š¿à C=¿Û|ÂHds¿ä+"Xœ‰¿âr¼Jž‰ÃAGNbll3FGL J0802.0+1005NVSS J080159+100535?ïüY5Ã[?1©›§^Pà?=7œÖG?1©›§^Pà?ïÆÕ&
?"-6|c\Ø?|•løt›?"-6|c\Ø?ïð€y?º‰?WÂòß(?Ÿ?^ÿ
œÎz?WÂòß(?Ÿ?ï}_;FIˆ?m'ÙíŒ×à?T"Ç3
?m'ÙíŒ×à?ïôåkedð?P£^}x?V5)2vpZ?P£^}x?îÀ}-Ó!û?°‹ãö	1?£ø-'cB?°‹ãö	1?ïêƒW™"?qshF¬2?e|©*ÿ…£?qshF¬2?ìØñ‡'I? sN£žwœ?¹8sÆÕ¹? sN£žwœAGN4FGL J0802.3-0942¿êi\\n¸@%çÄÁe~À9Ï6¿yÀ<#Ÿ¢È…@ 0ÊڄEt?ýî%\°Úÿ?¸ƒ|-""?¦Öñ`Lh[?ñ7¼šO¡ÿ@œ•.ûÁ¿ÕTúe
¿è‹Ëz½5€¿ÞßeUÅ¿Ù8I½¹3"¿ØϹü‰Ð¿æŠQýù•ƒAGNbcu3FGL J0802.3-0941WISEA J080215.63-094250.9?ïüë	=Û?/ÚP$?8§ß"§ø?/ÚP$?ïìÏÅ[®?qÿën^¿?c0:àǚ¥?qÿën^¿?ïñ]È)œS?oïO_5?]DoL'Jˆ?oïO_5?ï÷4ž¡?7¬nÁÕQ?Qèߧ@ÞY?7¬nÁÕQ?ïú|K¼'I?7ʇ¢í<¾?FÑ
p7{?7ʇ¢í<¾?…Ä‹Ç?–¥~³	e?'žž]?–¥~³	e?ïô<^ÄË:?h:`‰®²?W‡BX,ûU?h:`‰®²?ïã¹E[~×?YZeÅ`V?lFºÏPú?YZeÅ`VAGN4FGL J0803.0+2439¿çŽ'iä!@:»'ˆÛÀ;o"1zÌÀ<ºëªÞe|@ á:á}]ú@¢(ÁÀ)P?ÂX\›D¿¶YXê?ð·…Ýúòz@ýµ\Í¿":B¤â1¿âùóv"Á›¿äï:€.Ž‰¿í
DVq%Ý?܌%þpÛ¿Á
ôeB$AGNbllNVSS J080307+243749?žÑ"-?ż ø¼"?¦†¥«*?ż ø¼"?ïöea{'?S·X£…'Ã?S5=-˜Î?S·X£…'Ã?ïà³O‰fW?væcZó ?oL°"X?væcZó ?ïÿtÖÛ]M?ˑ7ôæ<?e*FºÃÞ?ˑ7ôæ<?ïùè‰kÏ?Kßë'd7?H]Ùà¸h?Kßë'd7?ïÑ1bš÷4?x´.}·&?wgNα1È?x´.}·&?ïÛ B?"?åÄØq!ª?roòMEä?åÄØq!ª?ïøû«ÿÅ?Ky¨§òTs?LOm–
?Ky¨§òTsAGN4FGL J0803.2-0337?r_!K@,b€àe0À9<IðuÀ<3{W3@=ÚÞ]mï?ÿ×¾³.–?ªu¾É?—Hº²™?æ—VO—î@	íÄoÜû¿³ÂA-œÆJ¿Ý!4ƒqý¿áwÂ^´Á=¿ÞæNþë­ã¿æÑE7Aµ­?•lÖÂïÔ9AGNfsrq3FGL J0803.3-0339TXS 0800-034?ïýûÀ$? ¬i<W¤\?0!þƒ§'Ç? ¬i<W¤\?ïðh`š'<?a➍‰?_/>Oÿ™>?a➍‰?ïõÊO¢ˆ3?[Ûíœf*¿?Tk`Lü?[Ûíœf*¿?ï÷ï_kAå?@¥""q7?P!@á½øk?@¥""q7?ïü%ٔ—?4[pxþs?>Ñ3Ô5ÔP?4[pxþs?ï±Fo-½Ü?k¶ÆöÕý?ƒ®d$i?k¶ÆöÕý?ïó0<ø?mŠÝÕºÝc?YùžOSÐ?mŠÝÕºÝc?ïî'YÈâ÷?SMÓE(}t?an¦8|àß?SMÓE(}tAGN4FGL J0803.5+2046?ïZV9adc@8ÉDg8~À;9Òïü|¾À<¬@ä@)°-ï#?ÿüS"¾?×7¤¨§ÿ?襢¡€è@	/ËOKE@
³Ë'åö??ïüÕ,ß¿­%ëbd#¿ä'§C¦Gþ¿ïÝu@ô¼Ö¿ïýè-{cN?ïpÿь$AGNbcuGB6 B0800+2046?ïüÞ…šè?@‡Ç1äì?9+ºøO–?@‡Ç1äì?ïéX0˜¤&?h꫶ê?f§Ï7QŽ?h꫶ê?îâF'Š?'ÌV7øi?¡Þ§ë–çc?'ÌV7øi?ïÇ?)êà?e/÷Içx?|`jöYhE?e/÷Içx?ïú	ÿ»À?V5ºÈ "?GØüü?V5ºÈ "?ïb"z•È? ¨6OD?"¯}-=ªú? ¨6OD?í}æþØ?¥Z˜ÉÛ-?´Ï^.Ä?¥Z˜ÉÛ-?îÄ\éeî?•?@¿GZ?£º1g¼ ?•?@¿GZAGN4FGL J0804.0-3629¿ÁC·dÛ¡ÒÀ á÷×<'À9ZÙæÃ1À;±¦Ùóü¼@ ¨%o{8?ú±À×ÌP?¹+³b¢3?Í/ö¨=vX@Ýð
¿w@{)(î5Ó¿èÁÿ)%¿Õ¶º¼©éô¿×¯[bQXã¿Ã(™|=h@¿áéñ€‹U´¿â	,«AGNbll3FGL J0804.0-3629NVSS J080405-362919?ïÛÃP³\õ?m(×;pŠ?rW¸ßi6?m(×;pŠ?ïÑdÔ,?'Úµöv?wMò±uÉÕ?'Úµöv?ï#ÍMŒa?"9Çï9ֈ?›†VP+¬û?"9Çï9ֈ?ïÓÃÊÖ¹œ?`A~z"U?v›'j
?`A~z"U?ïR>þ~²?•V%­aî?•®X¿Î?•V%­aî?î~¯Gx1?³Ä›ñÈ?¨‹ì‹C?³Ä›ñÈ?ì×sCeý­?©™Î@ìä'?¹Deãô+—?©™Î@ìä'?îþ¨ž^J?Œ]ىzà? vfý[?Œ]ىzàAGN4FGL J0804.5+0414¿æV>&ÆE@2.úÆ\À:a(	4À<U°i@íÊt­Ñà@œn`/ë€?¼q{BkŠh?¸LmbÁ?øNI¿f²½@
bK¤™'?ïýêa2Iÿ¿ãŒnØû¯8¿çÎÛ/f¿æú¤¬S¿èX<8d¿ïÿÈl뻥AGNbcu3FGL J0804.4+0418TXS 0802+043?ïýÖ·}c?"˜t驁å?1OÚÁmº?"˜t驁å?ïðnžTz'?anM\÷t8?_"æÁËì?anM\÷t8?ïé\<ù¹?híFuøX?f£ýó Ρ?híFuøX?ïíhy?GáT"¹öB?b~—ʉi?GáT"¹öB?ïúåèiO?AˆÔ
œ®"?Dh`ªëº?AˆÔ
œ®"?ïÁí$±?'g¡S/=?~}x?'g¡S/=?ï½_;FIˆ?€åwñ¶?€¨19ÄSû?€åwñ¶?ﲍµŽ?m]0ߨ;?ƒ\'À'?m]0ߨ;AGN4FGL J0804.9-0624?Ú÷›3û]@*Xä2DëÀ:‡ö'À<'õ»Ÿí@ ˜¢=W#}?üSd"?À©õ‡V ?½=ú·k¼'?þ;ýÝ@³6É?Ïy?Ð*ý$"®¿À
~ß06¿Æ"àå]'W¿Ü>&áì¿Ûm·_þ¿á¶óF´xAGNbcu3FGL J0805.0-06221RXS J080458.3-062432?÷M?¸/hN¾?ˆÛÅ«HØ?¸/hN¾?ïæÏüÆÔT?içµu‰I?i0Ò5?içµu‰I?ïãÓGõ?v«Î%ð†?l,¸Øì›??v«Î%ð†?ïÅ«#}?[5a¦Û?}*n`TW\?[5a¦Û?ïì—Që°?Wýhv?cïhå¢?Wýhv?ïW4ÜÍî,?œ'²AHY<?•dki¤l?œ'²AHY<?ï´9K·I¿?‰Bãoõˆ?'ñ­Þ¼Q?‰Bãoõˆ?ï2žÁTQD?ôüa%?™¬'ڝA…?ôüa%AGN4FGL J0805.0+6746¿î¢«Lä#@?䖚
Ø¡À;'çv¯ŠÀ=Ò®Že@¹+x~ÁÒ?ý3o~=Á?ÔJÙã5ÄÞ?ÜדdÌ2s@dZ˜Ó@ºŠ.¾³¿ïÿ–þߙƒ?ïÿ·pD5º¿À@˜ ¯¿ä<UxØY¿ã¬(|öˤ¿ïÿõƒ¥;ŽAGNbcuGB6 J0805+6745?ïüU5¼zo?89:…«¢?=VSV¢^V?89:…«¢?ïêP§?bðOÔí?e¯éz ¤?bðOÔí?ïiZ÷óA+?‰ÿfÀü¼?'Ô¡—Ú¨?‰ÿfÀü¼?ﶊ¦6µõ?d÷vu{x?']VÈÀÄ?d÷vu{x?ïúþ4í?Dsñ_Ü?GôØU+´?Dsñ_Ü?ï±òrg•T?ƒ¶øÛa¥¸?ƒƒcpˆÝ?ƒ¶øÛa¥¸?ï0Æ3«~?"÷ê1°Ê?™ç9ˆØnP?"÷ê1°Ê?îèK€±ì!?Œý9-?¡{Gð•ºù?Œý9-AGN4FGL J0805.1+7744¿ÍUžmýß@>Z<d4\ÿÀ:ƒ4-.6tÀ<{Wɼ@öFBÚp@]­Z@¾6?¹8¡ èÝ¿³éKó?÷5Ë(‡Þ†@Τ¬È"¿Ð"Ï£@âH¿âFó¤§ê•¿éçåWMÒ¿â©i»…|¬¿ê¦>"z~K¿ïõ¬EmÈAGNbcu3FGL J0807.1+7744WN B0759.6+7754?ïû৆R{?=Çç—._?@}aŠZ-M?=Çç—._?ïö[°?TYí0îS?SIþ™«Å?TYí0îS?ïØ	îZ*?wÏÊ´íӛ?sûØj\?wÏÊ´íӛ?ïüAäžG ?$çK¾ÆU	?=ðÙ'Ë;?$çK¾ÆU	?ïögnŠ]x?S#~S§ÐÊ?S1#¿pD?S#~S§ÐÊ?ïÓá¨?{7í:¬'?vrˆÙ`å?{7í:¬'?ï܄J|ûÔ?|HQˆÌØa?q½ÚÓ`
×?|HQˆÌØa?ïåTÑúšL?YI†‰'p?j«.ÄLB?YI†‰'pAGN4FGL J0805.2-0110¿í†'ºý8ó@/"(ÂzÀ9±Ç²±˜"À<,<{±QF@W¨—ä7Í@ÉË«d9?´"D•ÜÑ?Á½…\ @çüMÃØ@ ççÛF?vRdë€Û̿ݲ´Þ¤'¿ç¡&Ö-Ÿ¿æ
ݹ.4¿êö&B4¿ïÿÿ>¹úAGNfsrq3FGL J0805.2-0112PKS B0802-010?ïûñ[*%Ì?4¶d§~ê¦?@:'À:þ?4¶d§~ê¦?ïñ99÷6r?aɯkÿá¯?]Œ[ʬc?aɯkÿá¯?ïÙ7ˆú²[?p– M0j?sd;ˆÖ£?p– M0j?ïü(–2m!?&.ùëq©b?>»PBÊ ?&.ùëq©b?ïú;ämäp??ìt@]È^?Gm©_æ??ìt@]È^?ï±°£:F?‹§2÷] î?ƒ¿SË*̌?‹§2÷] î?ï'ñØRšŠ?ˆ¹jÙãl¿?‹ƒ‰çéÁw?ˆ¹jÙãl¿?ïòÙ1<Á…?H!®rŽþ¹?ZMÉÆ«?H!®rŽþ¹AGN4FGL J0805.4+6147¿àƒŽâ¨Ï@@.}ªOÊCÀ9ºi¨:FMÀ<e(wŽ'@k`ÊÆi@$>úè?µ¶e)O…?Ǟ^ºËm|@
k4*©ø@˜‡C'&¿ÏBi‡¿å¤ÇÛØX¿ë	øÂ!¿é»©Y*=Á¿î_Jé2^!¿ïY/±žsAGNfsrq3FGL J0805.4+6144TXS 0800+618?ï•WÚA¼?±‡énYl?Šª8'Y"?±‡énYl?ïõ§¼Çñò?W_Ÿ{ô€»?T°†ˆÙLŸ?W_Ÿ{ô€»?ï¥ÛÞì?ö'"¿U?†¾ý6Pä?ö'"¿U?ïý•Æ6–Ñ?!a=9øÆd?3QÎ"šãé?!a=9øÆd?ïÞ¬'ˆ&¢?l:ґ˜Pg?p©ìNz'ê?l:ґ˜Pg?ïÎî·G\?€ž1"‰3?xˆ¤aó1à?€ž1"‰3?ªÏU?˜ ®TÊY@?¤%>v.ñµ?˜ ®TÊY@?ïö­{Iû?CóŸ4ם,?R¥	ƒô+5?CóŸ4ם,AGN4FGL J0805.4+7534?é:é»èE@>Ëeºnü7À8áhSÀ;ÿ.Y°@Aé~3b?ý&ÈVE†ó?¡'ccý?™_»…iÐ?øéq-iŖ@Lœ«œÑ\¿×öÞN«¿ÕHåL"C¿ßÃcl‹ï¿ÙÏ¾ï"x¿ÛtúÓÆ;¿Þ¬Âû<ÍAGNbll3FGL J0805.4+7534RX J0805.4+7534?ïþȝñ Ÿ?êÍúƒn&?#v$ñ³x–?êÍúƒn&?ïõ¡S ?W8"Ø?T½Z@v¾Q?W8"Ø?ïög·Ÿ³?\»'éh
ï?S0'Þiä?\»'éh
ï?ïó¨+,Ôt?FPs^q­?X¯©z\{?FPs^q­?ïýº¢Ë?#¤•Ì×Á	?2*è3ÅGr?#¤•Ì×Á	?ïÔ4tYw?{g7­=?uùåÊ¢¸–?{g7­=?ïù&íŸÈ?]io˸ýA?KdJ«í} ?]io˸ýA?ïçû
'Ó?Z$f]?hö2ñtÅ?Z$f]AGN4FGL J0805.8-2331¿í¦vUæ@õĊÞìÀ:ÈlÁÊ:À<GÛZ.I¿@hÝao†¡@*':ƒŽ?Ç刚î®I?²Ë.'?îꀥ+ô?ÿÑɶÂÊ¿ïÏ@À£\?ïùåi{Ĝ¿ä(íßìå¿ãûØSÍ¿à-d‡im¿é¾@_‰ÓAGNbcuNVSS J080604-233333?ïü6Ãû0Ò?5ñJ³?>Iàe%ç?5ñJ³?ïË—™3?ƒÃbb:?z}4Kõ–?ƒÃbb:?ïí«ñyÄ+?T÷I¸
Á?bT™,Þ?T÷I¸
Á?ïÛǾþp?TÒb[¿l[?r õQ{ø?TÒb[¿l[?ïõ"zèBc?K¦"Ðv?T÷
ftùÞ?K¦"Ðv?í͑gé?Â?»"0@\?±"tÂmÏò?»"0@\?ïÞÔTçŸ?už0ÀYÒO?p•Õ~rí?už0ÀYÒO?îó3#
?:½Šu˜? ÌÍÍ£˜h?:½Šu˜AGN4FGL J0805.9+3834?ï÷[ùri¡@>o|¯Ý©À:¸""œÚ—À<ª#}@ëÇ8ä"@ïáÝÖ
?À5a¶©Iæ?˜â¬/t7?ÛIÝC½o@Ð2ÕÀ;o?Òïaz¿±>Y,3s¿æüz9'Í¿×ÙÜÀ4ãâ¿ßÌ´ðã¿ë—p"½'ÆAGNbllNVSS J080551+383538?ïþˆ™õ'œ?|‹9—?'v_}÷ü?|‹9—?ïö\b×e­?R+°à@®?SG:=öÖ?R+°à@®?ï÷š8Ùmù?T†A
Öڂ?Pˍê/Ov?T†A
Öڂ?ïúw' À™?&ù&Àª_?F!ºT?&ù&Àª_?ïýƒFy"Ÿ?+B]ÇØ?3åÎ=Ÿ¤Ÿ?+B]ÇØ?ïÔ+öJl?v'͐?uêüv+(?v'͐?ïûÓ®?U£e\:'?Cˆ±wgïP?U£e\:'?ïî$ÔS\|?Lý,Þ.¢ž?aÛ+}èÔ6?Lý,Þ.¢žAGN4FGL J0806.1-0458?ïþÞ
M+¾@,J•BCÀ;NŒ"¸'¬À<'"ØAu@mö¶@?ùéôÆ)?Ý
¦a©]?ì]d[Ø@§R°Å/@DG?"¥A?Í$‡^X¥Þ¿ïþßÙïÊÿ?ïÚ%`ÙR¿äŠÿ?:Ó¿â &`¼Ù:¿ðAGNbcuCRATES J080608.79-045411.4?ï÷­°˳?IƒŽâ…ŸZ?P¤Ÿ¥­ê+?IƒŽâ…ŸZ?ïÛ¥iþ÷?w™ŸÜ#`é?r-K	 P?w™ŸÜ#`é?ï‹áDÓï?=Aë?®Ü2+²?=Aë?ïN¹0¸¯‰?ƒ"gx°¦?–(Ùç2@Ô?ƒ"gx°¦?ïð—"ìck?cOFQW'a?^Ðöy¯É{?cOFQW'a?ïW¹œ»¯f?œŒÃa-a?•ÌhŠP?œŒÃa-a?ï.ñª?•ÃŽÝq?œ?ZïÊ?•ÃŽÝq?îjX}¼æ? Æ&ôÄ48?©Zx'¡2)? Æ&ôÄ48AGN4FGL J0806.5+4503?×-‡ùšFy@?«À~à°¯À:µ *­R´À<ŽIöÄ@&üª‹@ð×°´h?ÉÂõ³uã²?ÀT…h_9÷?óNcaÏ(@úŽ±´Ÿ?ïþrâÅB¿é]÷vĂ¿áJ
À2	½¿ìQµ(kY¿ïÿݛQ)¾?ïÑB*òÈAGNfsrqB3 0803+452?ïýÇXĒA?4g'mÕãM?1Å7ó?™?4g'mÕãM?ïöxö>"Â?U)~&• Ô?Sã¼P?U)~&• Ô?œ^µ?"µ@×4ˆ?‡^Ò	Þ?"µ@×4ˆ?ïû1ʵ?1F­ù³~d?C·;èV§r?1F­ù³~d?ïügä•?D‡ÚÆåâ?<ÂÄM+y?D‡ÚÆåâ?ïÑÒ³@´¦?zŸ7ôÔñ?w¦=ù'?zŸ7ôÔñ?#"*3?‰Øƒßÿ÷ ?‰X·AÄGM?‰Øƒßÿ÷ ?ïçüªX1?Y%÷1ý5?hV(&M?Y%÷1ý5AGN4FGL J0806.5+5930?êqûó€ë£@@Ig#$È6À:}Æp'9SÀ<«Ù§¦¢—@ ¼²MoŸ@%¥á¦x¥?·gŸïôð¿'¤üñz#?Ú}"ÛF-@£I€C‡?á¶Ì7«h¿ç}€H9Ö¿ã "IÖä¿à%°"±"¿Ç-\"H¿ègõ¢ƒøóAGNbll3FGL J0806.6+5933SBS 0802+596?ïþO~öÞ¢?B@¬?{ý?+<².Œ?B@¬?{ý?ïöcìZþ÷?WUgeìÐB?S8'6ÄC?WUgeìÐB?ïúã$õOD?6rYL0/?Dsk.llÊ?6rYL0/?ïýOõÐk?!¨"\H1?7ýøm.Ü?!¨"\H1?ïýRt¨.Ä?.Ž¸ßú?5l\·6ä
?.Ž¸ßú?ïԆM8z?{¹¯úß"È?u¼Ù'«?{¹¯úß"È?ïúŸwg7?Z«£þ; ?E'#;%¶?Z«£þ; ?ï÷U+?@ßW:ĔÔ?QUš°'Í?@ßW:ĔÔAGN4FGL J0806.9-2151¿ã·jaÀá@fð¸»À:ÞØh'À<m¹ô'ô<@dM¢JBC@V§ý	«z?Ê0mƂý?Áw$ºŸR?÷;º‹¨â?ø<N¿ÓÀ?ïì²²$«¿épà'ÒU¿äX§–²^Œ¿Ì\!©s~¿ë~o§WÈ>¿ÑAqºWCAGNbcuTXS 0804-217?ïöF­'YÐ?Qø"™J?Sr¦,þOw?Qø"™J?ïwݙp q?•™ö'—<Š?'LÑûñå?•™ö'—<Š?ï·â-m\¶?~ùø"Gð'?'t±jr?~ùø"Gð'?ï] ŸrK¢?rŠ²Çx/(?"Kì!Ê?rŠ²Çx/(?ïëf!êWï?að80Kãà?d™Þ/Åd?að80Kãà?ëµoÀy¤©?Áñk×X[?Á*@þm\?Áñk×X[?ï£F]Ä?†6?ü:?‡?îsâÝ?†6?ü:?ë²öèŽÛ?¢Î'9±ê?Á4'€]Ē?¢Î'9±êAGN4FGL J0807.0-6102¿ÑKØØÁ2À.¾ó'ªÀ;¤˜ÑÀ<ª^Ô¡­d@¦/ÕÔ¦?ÿÜÀ_×?Σ:Xš¡?×êÈ@ +š@F™&­ó@ŽªÙÝ×a¿ïÿý`éNä?ïÿþó…õ¿Þt—A$¸q¿Ö×=¾ýVW¿ëbÛ, Å¿ïÿöùŠpAGNbcuPMN J0806-6101?אַ$Ò-›?ƒºAX‡¤þ?"ÔvĕaJ?ƒºAX‡¤þ?﯉±€QZ?†ÒáJŽ?""šlIu?†ÒáJŽ?í™Ú.Š,?¡Ìƒ?³1.ŠÒ¸f?¡Ìƒ?ïa ÃHXx?tXæðÀ??"ËçœZó?tXæðÀ??ïjx+¾R?‹Á´•ø?'®Pó¨ý¼?‹Á´•ø?îj^²Và?µi‰Ž7$?©ZړÆ?µi‰Ž7$?ë)a×F´?®\Ú‡?ÃZx¢å-þ?®\Ú‡?ì!¼¥"«Ã?©|½øRõ?¾òÓÚ¡æ?©|½øRõAGN4FGL J0807.1-0541?æö­qùÓ§@,VߋÀ9Š]ÜTÀ;³›ý÷è@v©÷	â,@ÌúÕS"?«ã!€‹ß$?¹"€z䢬@
 sÃF;N@
¶áQê?î¦xÚÝ0È¿ÖE—¤Kú)¿äp5݇…¿àaßyw»¿åþw4ÿì6ã¡¥¯AGNbll3FGL J0807.1-0541PKS 0804-05?ïýYkšòy?*²oq±ð?54¢³ßßs?*²oq±ð?ïŽí]?g=˜û|?adO`"ƒ?g=˜û|?ïޖÃüC³?tÜCKOýÎ?p´ž
r‰?tÜCKOýÎ?ïøÂ.Á½?1Õمm-=?L÷DÉŒA?1Õمm-=?ïýëÓº^?(rþJǵ‹?0¡g²Ñ¥"?(rþJǵ‹?ï7º\f?š¤èτ.›?²ƒ·ºT?š¤èτ.›?ïȌ~S)?ƒaŠuÉÏ?{¹ÀËu«q?ƒaŠuÉÏ?ïéÍRûòÍ?PƒÇ["ò)?f2¬þÓ?PƒÇ["ò)AGN4FGL J0807.2-7630?ïºKLHqÎÀ69†3‹HÀ:‰: >BÀ<pâkš'Î@ÁnØå@î€F}?ÃTAöš{—?µªZ±ý>?ò0œë]±Œ@	ÁŠŒ5'ï?°	/(·";?ï lf±¿â-颛uè¿áª}?Æ¿¿ãt¶‹Aè¿éiõ1oä"AGNbcuPMN J0807-7629?ïþ•Q‹bõ?õPú|ƒ'?&ªçuË®G?õPú|ƒ'?ïõ ÆýˆŠ?Y(í‹f?U¾r¬Ó?Y(í‹f?ï÷kûëb(?<ÌŽlå?Q(9¹Ïå?<ÌŽlå?ïù0"ª?0õsNŸ&ú?I¿?Í_ç?0õsNŸ&ú?ïýÓ=\à^?%ÙÅÙÙã?1fdÚÓ@?%ÙÅÙÙã?ïá)æ%?n‰@gÅ}J?nê蘭{k?n‰@gÅ}J?ïø ¯?W±Ç^¶@?M}ø£`¢[?W±Ç^¶@?ïìT"/F?TLӒâf?c«|NÚ	?TLӒâfAGN4FGL J0807.3-1954?éÃëUN@Ôó…À;e*ýÌÀ<r»H@
²@ØhOõ‹³@V—:*?Ë"-;øS¹?±åޖ£Åí?ëV—¼IÇÊ@Ò¡ÍðŽ?ïï"Ê/d¿ä6A¥¼½‹¿å²>àæ¿ä"8säÔ+¿ÔUÞXæK¿ã!ÂUO"AGNbcuNVSS J080722-195218?ïý‹£" ƒ?%%ÈU?K?3¢â/ù·U?%%ÈU?K?ïæۚ1T?o	ò	VǶ?i$e'{É?o	ò	VǶ?ïðápŒžÎ?V)y½-?^=é'±?V)y½-?ï÷˜Þޝ?3Ø3Œ?QÚÍâ
¶(?3Ø3Œ?ïýoJZ?+LÀͱ6?4…¯?^?+LÀͱ6?ïPjüx6?¦¯ëÃòƒw?œuò§P13?¦¯ëÃòƒw?ïï›À%i?ja-Áy?`d?Ä2îÄ?ja-Áy?ïÄ/ò'?mJNµŸ#'?}ñè#Ž$C?mJNµŸ#'AGN4FGL J0807.7-1206?ï!	±ÉU
@%ÂÂ7G"êÀ:~[ãU¥À<;yQ$µÂ@~!IÑ°6@K>WS£ì?ÃæÆÞvB|?ŽZYñ@¨?ÆѾ¿@	è,B©ï¿â®˜™¿YG¿ç²Á-Ý3¿ç[bA=·ñ¿é8'â3n¿åõæ×:¿ïÈc`øh\AGNbcuCRATES J080736.06-120745.9?ïþóH•"Å?Óú.•? Ëu‡(d"?Óú.•?ïïú5™P?b)¸¬u'—?`rðâOœ?b)¸¬u'—?ïóFÍމ}?GÊÇ(´$'?Yrd|¦v¦?GÊÇ(´$'?ïþAúÔЅ?@ì›o?+àQ%ó(?@ì›o?ïÿn"¦>?u‰;ú¡?-ƒ
çy?u‰;ú¡?ï	)Á¼Æ?–!¦Fdä?Œ=µO>~?–!¦Fdä?ïîÜí‰äM?d†YÉf)?a#œ—RP?d†YÉf)?ïöÃ(7?D'û3ÑÉ?RyùÞ®A¶?D'û3ÑÉAGN4FGL J0808.2-0751¿î¥WIë@*R¾H¥‹?À7‰²gƸ·À;Vd'PÐ@¸éö©?)@å*"8…?•e‰Ç"~¨?µR3S"|¤@ jvSCsó@¸[äWX¿Ä®YڑÜa¿ßÃt
6¿ãk–¼o‡w¿ãž4"䤿æï9©nù³¿íRuÚAGNfsrq3FGL J0808.2-0751PKS 0805-07?ïú9fú?CÒàtOD?Ggƒ¦Ã?CÒàtOD?ïÃT'ãÓá?'€Þ£3ò?~U·D–?'€Þ£3ò?ïÐÁ_A•2?€
?±V[Ð?wŸPfŸ?€
?±V[Ð?ïýً2^Þ?(›FàÁ£²?13§Ã[+?(›FàÁ£²?ïôxbgSK?SÓ$øVl4?W;ªK¨«?SÓ$øVl4?îÒËñIrª?±©'}·	?¢Ó@îØqc?±©'}·	?ïÑ çV:õ?"
®Ä ?woŒKó‰}?"
®Ä ?ï÷́ð§ë?E5ö¥Íõ?Pfûø4ŠÆ?E5ö¥ÍõAGN4FGL J0808.5+4950?ì}&/Oßø@@EA [ÀÀ:
é¿KÚÊÀ<n«ï³x@^'€L–‡@¨1­!5Û?¼µ#7èz?¾Ô»-½þS?ù‰žsóî@©A,p ?á?ž{«¿æ¶<½u–Û¿éfæÀ¿ïL´ÔQP¿ïüð¡=Qð?ïûûùáAGNfsrq3FGL J0807.9+4946OJ 508?ïý¥$ð­Û?2gÒ2›¸˜?2Ö؃\ó«?2gÒ2›¸˜?ïï	{åå´?a|¡çr÷¹?`ö"ºtM?a|¡çr÷¹?ïØ&°ÿøÚ?yÑêx™@Ç?s짋²>Ä?yÑêx™@Ç?ïÖöìÛàç?bT¨*ƒo·?t"‰{b ¯?bT¨*ƒo·?ïër&¸ü`?kï=Î
à?dÙZAo'?kï=Î
à?ï—sÈù6?"·-CÔø?Š#<CrÞ~?"·-CÔø?ï°ªYÁy?…™²R©ïH?ƒýÕs†Ì?…™²R©ïH?î[m°Bä'?ÓÂ]¨¿·?ªI$ûѶÛ?ÓÂ]¨¿·AGN4FGL J0809.3+4053¿êº˜6)@?""åÕ²OÀ:Zi¡"I¦À<yèÿ2z§@ög¢{•x@ü6ڇ s?Á¨wB¯Ã?ºzÈH-Á.?÷ oz@
6H°HÕ?ìø´¢¨ñ¿æ6¿áa¿èׄKS»i¿ásï@j(h¿ïÿð°×£À¿êëÒ¶ñ™5AGNfsrq3FGL J0809.5+4045S4 0805+41?ïüô5$?@€×à¹2?<‹#?@€×à¹2?ïô֍ÖÔ?W¿q6zm¶?VSÍ#‹'Â?W¿q6zm¶?ïéÕmt?h.æḤœ?f*'S•Ût?h.æḤœ?ïó 
Ìâœ?A¼~«	ÜV?X¿êšt×4?A¼~«	ÜV?ïýjåY¿?3?P	œ"Ã?4¨Ön°s?3?P	œ"Ã?ï΍,V}Ä?×Zã-?x¹iÒn-?×Zã-?ïó/È£%?aAæ
}¶?Y n¼uˆ?aAæ
}¶?ïÐÑkX$?d]ÂvZ@è?w—uÑ3&?d]ÂvZ@èAGN4FGL J0809.5+5341?ÔQõf‰@@vQ ÄeÀ9OM½øôsÀ<w^o@ÿ½ð÷4@QâZӋ?®2ó'Þ?¼ç—~aYâ@¶î·`-@
+m—C¿á+}âƒî7¿Öļþ"°.¿ä­'Lž>¿â±4Ur"\¿è"âÀ*'¿ïÿûbâMhAGNfsrq3FGL J0809.5+534287GB 080551.6+535010?ïûÞ­Acš?7£êâ½Y?@…JùX}?7£êâ½Y?ïôþ·"
?Xâ‹N÷å¢?V'7ôÛ®?Xâ‹N÷å¢?ïԆ°ïݯ?t'·¤Záx?u¼§¦M¸??t'·¤Záx?ïÿ™Gä?
,âMí4?,Þx_Ÿ?
,âMí4?ïûÜâ.Å?<قÆLÉ?@€f:t?<قÆLÉ?ïÏl›{?x¾Æk^Ì?xI²ˆfR?x¾Æk^Ì?ï¯w›†Èu?‡#©âÃØR?"")L¢–?‡#©âÃØR?ïýÓ§¯ÿ?#6C&¥?1gŠØ}†q?#6C&¥AGN4FGL J0809.6+3455¿ÛhC"Ü@>[=ÀTïFÀ:—öÀ¼RÀ<…¬bäÒ@ ìKœ%?ü­,SE!r?¹½0EÃ?xHÝ%Ï6?±o¤'½@çèF¥Ö¿?ï…[ôó]?Òà™ËW'¿ÝC­iZ6­¿Ô
ÿx›¿åOoù?·î÷€:ß
AGNbll3FGL J0809.6+3456B2 0806+35?ïþˆ˜â±Þ?áø`Ú®õ?'vt[ekó?áø`Ú®õ?ïõ{{»& ?S…ªa°y¦?U	§ðO®?S…ªa°y¦?ïöšm¡e?\.ÖTzs–?RË%í?\.ÖTzs–?ïóŠÿLü³?A_`ñGqò?Xêø¼?A_`ñGqò?ïüÙL†?2,áÞÅ©€?95ž'Ýéç?2,áÞÅ©€?ïÕÓ±øŽ?và+
p?u'_ƉD?và+
p?ïùi.Ü{/?\µËw6ì?J[CûJYž?\µËw6ì?ïè
.$?UUñÃ*?gò~çÙnú?UUñÃ*AGN4FGL J0809.8+5218¿îó7æÝUl@@uÂôÀ7ßF€"À;WFG.@ѹ©™è?üúÜà@G?™úAú÷,? ¯·=C'a@Æy{ìài@/®'MoÊ¿ÈKÇ©¢PL¿Û ÿ-C¿ÝùVÆ'!¿Ø`Z³ª¼Ø¿à҈˜ÀUÆ¿ØÿŠÄê€<AGNBLL3FGL J0809.8+52181ES 0806+524?ïÿ9ìú"?œ Væ7¿?8»ê ?œ Væ7¿?ïö8›ÒÙ×?T—ÝÅ)'´?SŽÈ²BQC?T—ÝÅ)'´?ïí	TPf?hÊmL`¸?bö«"MA€?hÊmL`¸?ïÿ€oÀÆô?=ô[þy?ä,@•?=ô[þy?ïþ+¦:ք?#ÅÛêd?-EŸ€;4A?#ÅÛêd?ïÏpzV?€*'ÙÊ?xGú›_=
?€*'ÙÊ?ï讳ÃM?s'xÊTj?gçQë
?s'xÊTj?ïÿ–iŸ'?Ú@í»09?
eŽ–²M?Ú@í»09AGN4FGL J0810.9-4926?妜bKÐÀ!8÷‡‹zÀ:·SŽÕÀ;ó¥è\uL@'ªk¤@K€œr'î?Ìw›Žy?¯ðRAâ?äSõ`æè?ყòͽc¿çµfI
5
¿ã݄ªõ°¿é…Áàà€¿Ý8Îø ¿åÇM1:Ç¿ïØ¢žP³AGNbcuPKS 0809-492?ï÷u¿
¶;?hã½ïÚ+ý?QªÚ¨?hã½ïÚ+ý?ç€F%?¬¢ñqD?§‡û¬?¬¢ñqD?ï—äOö7?Š"!ޏ&?Šëû'è7?Š"!ޏ&?ïTƒ˜ƒø?""ÀJ†¬š?ŸUo_ì?""ÀJ†¬š?ïè5¢½ô\?rÆIÛØ6Å?gÊ]q¼ª?rÆIÛØ6Å?æB"¦å©à?м25\XF?Ózö²4¬@?м25\XF?ïX!7f?Î^ó*"Ž?"ý=ùÛO?Î^ó*"Ž?äP)ŽÝ?¿P¬š0?×Û_¬ãÎF?¿P¬š0AGN4FGL J0811.0-7529?çoÿ×¼À5r=_ÜßjÀ8~é°2bSÀ;ŽÅ=jÅ@ÎȦ!'L?üûõ)hÄ?£pî!'ºQ?³@ÒÙb@{Sþ"Õ½@	.¡Kϖ?ï`ø0'æ¿ÔžÜÏyOw¿Þ_
agy¿Ûé¯Çˆp¿áD…Àô§\¿àW}à€ˆÑAGNbll3FGL J0811.2-7529PMN J0810-7530?ïù{'›ÉJ?J–\ßvӚ?J¹ÇGÜ?J–\ßvӚ?ïØÌ-ü¤?tY"nà9?sýÊ2M?tY"nà9?ïÓªa	|£?}H˜.hP?v*ϗnzi?}H˜.hP?ï}5°ï2?t§í4@b?YIÛ0áÌ?t§í4@b?ïä鹗Ö?j>¦Eôm?kF,Z
?j>¦Eôm?ïF^´ã™?¤"»œq:?—>4,Ó(Ï?¤"»œq:?ï€
¯bó?'¯€ó	?üº!å³?'¯€ó	?í'nØáê?›kQ´\üK?³od‡/2?›kQ´\üKAGN4FGL J0811.4+0146?æL
ô6ƒ@2ìAÝ"À8ð&n(ÓÀ;nÇtž8@G4 ñ|¯@üÉð?˜ÿjÙ½¡?±ž
áXä·@]û¹I@³¥ÂqÕ¿ºž'úb¿ÝxÞ8/¿á¦.ÓR"¿à· ÈÍcÌ¿æHùµ¼æ¿âD`ý›Ì¥AGNbll3FGL J0811.3+0146OJ 014?ïú¹ƒT?@\ºûoö©?EbRn¸?@\ºûoö©?ï텤š(¶?rˆþ|¬S?bz[\8bb?rˆþ|¬S?ï熮ҳ8?kôÑhßÝ·?hyPù¸+?kôÑhßÝ·?ïþC˜õ?¢Lµ
@ê?+ÎZ€	È?¢Lµ
@ê?ïüxàÖ2ì?2Rd)¶äÙ?<8÷-
¸?2Rd)¶äÙ?ï¯ïè–èö?Ž¼½²"ì?"ʘ?Ž¼½²"ì?ïé
T0›?wâғ¥T´?fõ«¹dä©?wâғ¥T´?ïûÚ\`Ø?4Gò#"•›?@–GxVn?4Gò#"•›AGN4FGL J0811.9+7847¿ï顦¥¾
@>t‰ãC0×À;Z¨®àR¼À<£¿Ü#å@úËܑ¼?÷Ud;ü?á"r&Ž	?æJ 'l"@Ž{Xeó@gî¸/ý?ídIáJˆ9¿ëÇ€\±²¿Áã˜ËéM¿æ¤á@¢1™¿ïü#åGî¿Óè5=ÏnhAGNbcuNVSS J081307+784308?ïò^úÝL?^²î,(Š?[Bb¹†"?^²î,(Š?ïëæ,5r?aÛ:¢?dÔ7]<?aÛ:¢?îäy¶ád?Ž%༾™?¡·(`FfÂ?Ž%༾™?ïtÊ}ÎH?vˆ"G%ž?'}F±þ÷?vˆ"G%ž?ïç㔘£?o¥ƒ)äy?hk™t¼[?o¥ƒ)äy?ï©tI—½e?…¤Ãdr?…¢í«>²˜?…¤Ãdr?íúmìã™? õ¡Gþ)?°,—¹Ö»? õ¡Gþ)?WÈ?"²Åôó/Ù?¤^öWü†?"²Åôó/ÙAGN4FGL J0812.0+0237?ïçk²ç¯@3ÚãæÄÆÀ9ðËЮÚÀ</°r#3@ Îý~›f?þÝΗ¨'Ò?¶Éš'ª·¿™UpŸÐ?s?㝺|h0?õ ôg˿1f™'?î
üwµCC¿âÆAp㘿Ù*»*
Ä¿àcJB~Q¿Éy—›'˜AGNbll3FGL J0812.0+0237PMN J0811+0237?ïù4;hXP?C2›%SÉ?K/ÁÀé?C2›%SÉ?ïʵ`Ó,?†'¢Õ,˜?z¥O¤:ÙÜ?†'¢Õ,˜?ïÓO-ËÑ?v_ôÙ ;?vuXI}¯|?v_ôÙ ;?ïk‰UԝÒ?{få<?'ŽÕ<Õ?Ú?{få<?ïîa?
+þ?X͗­›+-?ažÀôt*"?X͗­›+-?îå-5('?±=!õ»[ö?¡®í0Û?±=!õ»[ö?ïË2
C_{?ž§Õª?zfù] Vd?ž§Õª?í¶WÚ a?¦r¨R¿Ì{?·úMCT¾s?¦r¨R¿Ì{AGN4FGL J0812.3+1143¿æ^¶!m@©@76OD
ñÌÀ;«°óRsÀ<‹Q$µÁî@ͳLóùŒ@ÞÖ4T›c?ÎAƞàUk?ëqÈÅ+C?ñlÐÈÚÏÅ@±´›Ó†?Öñe]|ÝÌ¿ÔÿcÍÚ¿¿çût_ÎFÊ¿ä#@v蕿ïÿÉ
ûkF¿ïÿ–þߙƒAGNbllGB6 J0812+1141?îc_ƒHIp?Ê¡²ºï?©ÊÉÛ?Ê¡²ºï?ïî/49Ý5?`Þ^®ÚÉ
?aÐËú\Úy?`Þ^®ÚÉ
?ï»wvÚá?w•t'ïFw?""JÊ×ê?w•t'ïFw?ïÙÅÿ±¯?SGӀk?s9x0?SGӀk?ïíÏHÓœ?\œ8‰*?b0¶ñäk?\œ8‰*?￞&­O?€øœ3ÔÐ?€vU´ì?€øœ3ÔÐ?ï-AU¤'?'èúµ%VË?šWÕGþBý?'èúµ%VË?ï7Ž•7=?ƒ5a½JÚ?ž9)é|i?ƒ5a½JÚAGN4FGL J0812.5+0711¿à
½S©d@5LP&‰ÅÀ:Ë7š¡–À<qe/.Á´@wP3:@
¸A$?½µ˜'ԅ¿‹R"Sba?ÅÀ›{œª@ˆQë…¸?ÛÏa×`z¿ë¢ÎLT¿æD‹ë[-M¿àâ4½÷ÇÍ¿åŽ)Þöšü¿ïÿ¾úAGNbcuMG1 J081238+0712?ïþËÐ"—°?áV6Ä?#C&þ?áV6Ä?ïõLDžŒë?W¡‹З?UgvpoŠÅ?W¡‹З?ïô'QâÜë?[˜1òŽÐÚ?VÛ\`ÁÊZ?[˜1òŽÐÚ?ïýb³ËÁV?`éAŽ°Ž?4êc0°æ?`éAŽ°Ž?ïÿ*Þ2?›<"ß.?½4Û'N;?›<"ß.?ïÕGfŠ½M?w™ÐÁd	?u\L¯¢™Ä?w™ÐÁd	?ï¦O#?fê®N.z?`m~̤_?fê®N.z?ïó§&ŽÏ?Iüș½WÎ?Yâ±÷š'ø?Iüș½WÎAGN4FGL J0812.6+2821?æ,IqZ'¥@=9Ñ쒛À:ö ‹Â[À<¨7Üæ @ƒ	ðï–Ñ@&÷ãÑÌ?¾r`ßW®¿¨õF'_/)?îA|7@èÈ€ÿ?ïåÔ`Û?ï½ö¥ä*·¿é˜+ˆ¿ãz?–îÄn¿ÊÓ_ãëL¿ÔÏÞЏ²AGNbcuRX J0812.5+2820?ïþÌùÅÓ?aØháD?#0iÏ9?aØháD?ïõևûP]?TW°n¤?TRðö«?TW°n¤?ïíE#†Ô?ppŸ#k÷?bºÜy+ÿ§?ppŸ#k÷?ïü£U?&DPV—ƒ?:ç?¬¼0?&DPV—ƒ?ïþ4©³uÁ?(¿%R	ÿv?,µhql˜Â?(¿%R	ÿv?ïÎtЕô?|¬
sÅV?xŗ•Ýž>?|¬
sÅV?ïðûÍÓ?o~ZÜ?›?^Ä	À*J?o~ZÜ?›?ïðµšJÍ?U1ï—Ï(k?^•æȪµí?U1ï—Ï(kAGN4FGL J0812.8+6507?ïŽÍžaˆ@@y§~^ª°À:žÌZ·»À<š€ÑK·Ž@ 'Íút@wßÖjÛ?¿kÂ_¥Eä?ŽŸj~y?ÐîOá?@>!œÀ–?î)Ý´{/¿èÜÏ^w"œ¿à'ä¾Ûó[¿ä"¥¡º¥X¿áԦ˱D¿Ë7Qzñã³AGNbll3FGL J0813.3+6509GB6 J0812+6508?ïúrJÜXl?7îRÈ¡?F6ÕK/D}?7îRÈ¡?ïô˜é ?U–ôIýÐ?WÌÎ¥ï<?U–ôIýÐ?ïïô¯"Ø•?aа‰Û˜?`P{¥‹=?aа‰Û˜?ïá
=èæ*?Rìog\~³?nõÂÚŨ?Rìog\~³?ïðW°.ö&?TZ;Ý<5Ú?_PŸœ"S?TZ;Ý<5Ú?ïф²VÔÎ?v»­œŽt?w=¦»(}'?v»­œŽt?ïõºd?o­?bøÈt욬?T‹7§œF´?bøÈt욬?ï†8¹YþN?v§¾¦F?ŽqѦÐ|?v§¾¦FAGN4FGL J0812.9+5555?Å7‰àg@@»3ÞLQÀ:þ'œ&;ÔÀ<¼MÑD*Ò@ ž
Lµ@CHÚde?ÃMИ^[*?"V±^ÿŒ4?Ђp½Ø=C@Àõܼ?ê80Èõ§·¿ç_&DÉ¿æ€(^ÃÚ¶¿×ì"é0°¢¿âBÞ¡áf¸¿ïÿ¦¶tFAGNbll3FGL J0812.9+5555NVSS J081251+555422?ïþ›ÚøšÂ?ýœmD®?&BLcý–ì?ýœmD®?ïöÜ"ˆÊ?S'íf–©"?SÎGOº^?S'íf–©"?ïø¶rmZÌ?<Ü1´.l?M&6°I>!?<Ü1´.l?ïùæ"ûÓ~?*h«-bΘ?He°ç¦c%?*h«-bΘ?ïþƒ\êo?"8iN«ˆt?'ÇçGá?"8iN«ˆt?ïصcN®å?s+ý@Qd?s¥NX¨¨?s+ý@Qd?ïùþRo¨H?WÐÕËL?HµÖ+a?WÐÕËL?ïì\§Rú?Plù"ª?c£YH-€?Plù"ªAGN4FGL J0813.7-0356?ïò¬?Ž‹I@0Jò"z–À:Ê/•ïÀîÀ<p¼Åd@!T(Ì'?ú{¬\ë?Èôî~ù/V?Ç`1Ùkì@J¡äÁ¶@;DI[Ë?ÔC¹"4$Ë¿ålüþóg¿µ…(ÞÆtn?·)£dm­¿ßüEá5ºw¿ç$8YáAGNbcu3FGL J0813.5-0356NVSS J081338-035716?ïùÝX$/?=úz'vrñ?HŠŸn<?=úz'vrñ?ïãH4Â?l6ÃêZ¼?l·ËW¥Š?l6ÃêZ¼?ïè|µÞ?cËÈ´Û?gôƒh^qþ?cËÈ´Û?ïÎ;æúº5?Y§¿Ø¸µ^?xâ–¡‹?Y§¿Ø¸µ^?ïôDÖÙZ?M`ºûkJ?WvS[Ù,õ?M`ºûkJ?ï|"èn?š¸µ'r$y?}۟ŽÖ;?š¸µ'r$y?ïÜð¸Ü¢O?s²ÐÇ4Ó?q‡£•Î`Y?s²ÐÇ4Ó?ï?!>¥=x?ƒ¶Á¨˜?˜Ø-?ƒ¶Á¨˜AGN4FGL J0814.2-1013?êË~Y"é@*m¾]ž@ÈÀ979_JÀ;ødÏ@ûÃ	€@•{âÏm'?¯©¨|Ø»?©^v¿
R¥?ú±ÅÅqŽ¹@	½Õ{G"?ïÿÿÊPË¿Ú$'óÕz¿áÒ¢dCvw¿á$Øâ"Äö¿äŽî_ċ¶¿å›«–òAGNbll3FGL J0814.1-1012NVSS J081411-101208?ïý°¿rh ?#擭Øó?2z]V\¿?#擭Øó?ïî'ÒWÑ"?b'°™ŸÖ?a}-ãH%g?b'°™ŸÖ?ïï•?ƒ1?jú*Oý?`jÀ³!÷•?jú*Oý?ïÞá¨|?ZªÿïUå?p|"æ8?ZªÿïUå?ïý$ԚÄ?0Å°ÒÞó5?6ßX²ð50?0Å°ÒÞó5?ïƒÔO€¤?˜æ'¡5˜‰?9
å@žò?˜æ'¡5˜‰?ïêíizm?oH×98Ì?e–@ÚÌÑ?oH×98Ì?敏kzwj?t)ó'dçë?…Ÿ¥Qr?t)ó'dçëAGN4FGL J0814.4+6926?ÌBUèd@@C3‡	WÀ<0€sWæqÀ=+ˆlJ«ö@"òÌ!V;÷?ú	‡¶Õë?Öxë8Ȟj?É¡ú{±§,?öD?Àà0?ÿƒµl3¿ïýv¸ÄL¿íEIJ̬ì?ïþä­³,?Ë¢Ú`S¿ââÝ°IßG¿ÄC/ÀAGNbcu1RXS J081407.6+692549?ïúÍñ1}s?A3ê6 ó?DÈ:~'¸?A3ê6 ó?ïñÕÒÞQ?\*jLYµ?\T[¾ÃýÍ?\*jLYµ?ï¼AvJÙ?'8Çs¾1?€ï¢f$'Ï?'8Çs¾1?ïጋOe)?`¥EÚÓs?nstŠ7?`¥EÚÓs?ïûò8Zÿ?=©nÉš\?@7¦´¯u?=©nÉš\?ïÊl׈]?{æÿÍ°ðt?zɔ0À'|?{æÿÍ°ðt?ïØÃsN?} M=Џ?sžF?hx?} M=Џ?ïŒôî\?†'<ø
D?ŒÂÄaù'(?†'<ø
DAGN4FGL J0814.4+2941¿á?"hk›@=üGõbÀ:õl‰–WÀ<'@Þí`Á@ ³»Öƒó?þí@ÅÂíP?ÈcF¡Oš?²b["Ñ2ã?êÛª ¨»?÷*&ˆó?ïþР@ý¡¿éËßR,¿Ú¾/Gì(¿Üè'¯qr¿à姏%¢¿Ø¦á€¸øAGNbll3FGL J0814.5+2943RX J0814.4+2941?ïýãë¢O÷?(Ý­ì÷›?0à¡>~¸?(Ý­ì÷›?ïÞÙ8YÒs?p¸¼†ö½?p"cÛUÖh?p¸¼†ö½?ïélipî?f»˜g­rÆ?f蓆ò?f»˜g­rÆ?ïšÖfb¤?iQ¢—§?‰Jzw•bÓ?iQ¢—§?ïýÔÆ[ç?,»|"zÕ?1_óÌœ?,»|"zÕ?ïn®´ç[w?›ŸO™£Þ?'*)f"-?›ŸO™£Þ?ïç*¤¡èü?s<õ¶g?hÕ[c–cí?s<õ¶g?íº—Œ_Z•?™>
h° ?²+C+Z?™>
h° AGN4FGL J0814.5-2642?áÖÙoêÀö@ªžåXµÀ:Ç!—)|ÑÀ<=ŠV/·~@tÿKû<@a$z2Ì?Ï«b"Y–t?Ó½Éd7
@ SŸºE@\—rÍÒÜ?ïœø^Kò?ÕÖ\îm†¿Ü±,]Vl¿æ«Ý¾â~e¿æ'ÃÉf¿ïÿÚ`‰,ºAGNbcuAT20G J081427-264422?ï'Ü?]Äy(wMØ?`QG[Ì?]Äy(wMØ?ïÄçV™?'òßýGf6?}ŒUñL?'òßýGf6?ïŽ'"³Dª?"4S+dŸt?ŒvÚ
f?"4S+dŸt?﻾—ª×?_)¡$*"B?Z
?_)¡$*"B?ïî.üí¦â?\Ì|á£+½?aÑéÎ8?\Ì|á£+½?î/VX7ŠÂ?±'­Š<?­
šÝ?±'­Š<?ïIˆ_4™?"O(Z%á?Ÿ6Îúø¤Ú?"O(Z%á?î­Â…µü?‹ƒæ5íV?¥#ØìÒF?‹ƒæ5íVAGN4FGL J0814.6+6430?äiÆPÿw@@šb=ú	À8©ƒEW"À<µê28a@>Èáè@Á£n.±Ä?žíC\B˜x? XÑÓFäk?þvk+Èç@/¢ÈÂQ¿ßLVð§h¿ÜgÇúÕô"¿äuð²…"ê¿ãsÉü7ô¿ä¡^E°Ž¿æ%ÜÓ«
_AGNbll3FGL J0814.7+6428GB6 J0814+6431?ïþ½«zJR?™Ô°Íÿ?$%Iò,¤Ä?™Ô°Íÿ?ïöÍ-è?Qþr…[Ä?Re¤àÌ<?Qþr…[Ä?ïëu´.'²?t€ûQ\"?dŠKëŠUð?t€ûQ\"?ïúU÷Xfž?<pòhۙ?F¨#óI?<pòhۙ?ïýéQŠ-¸?+>5Ciá²?0µr'%&z?+>5Ciá²?ïÓ\¸µ
0?}ÝbN¦ò?vQ£‡îD@?}ÝbN¦ò?ïØÙÞ¶·À?—-ŔV?s"«ƒWâ?—-ŔV?ïô˜>w²?T9øîÚ?Vτnƒ{(?T9øîÚAGN4FGL J0815.6+3641¿ȩ̂çÚE@?ì"F{åTÀ;ÿ!³®ïÀ<˜­4
@-£ôfnÊ@[¡/?Ê_d©ø·a?·oÇäÌÃ?ï2 Ñœ?f?îÅ.S-,<¿áBÓNÇ
p¿Ë@%	#ë¿ê¸¬"Wé¿ÜÕ¬˜¥¿æv¯Æ+É¿ïþϞŽKAGNfsrqOJ 320?ïùsmyÄ×?NÖÛ)Ž<?J2I2"¢Õ?NÖÛ)Ž<?ï'ÓIZ'?žc~<Œq?›–Ù%Ã?žc~<Œq?ïª7üƏœ?…KrÒ×ê?…rÑ˵?…KrÒ×ê?ï
YÞ~â?€Îy¾›?žTÄ7ôÈ?€Îy¾›?ïë`Õ>«?kÃG—¶?dŸ*°]\?kÃG—¶?é6£¹
Ö¦?ȽK®ìŒ?Ë%qÔ¥g?ȽK®ìŒ?ï|ïã¹^—?AÒý N@?bˆÔ-?AÒý N@?爜¹"?µ@Ÿaƒ?ÐïÔƍºá?µ@ŸaƒAGN4FGL J0815.9+2951¿ã½S4Qãš@>VΚ,fÀ:ûàÊ°'ÚÀ<q±6nQ@E´%¶óÈ@zvSCsó?Úz}ib?×r2aüõ4?ÿ‹µÆ 
b@Ùèú)ý*?ïÿ~‹¡3¿àLÞÕãÍ¿ÔôŸd3Ü&¿è¤N"áÉ´¿ïþ8µS3"¿ïûÀj¾º»AGNbcu2MASX J08153642+2950218?ïÈ(ön[Ó?€?i‡æ`?{넩嚎?€?i‡æ`?ï×ÿ¹fÇ?z)k¾$øb?t#\jªê?z)k¾$øb?î¦\XèÇ?"²±hyX_?¥ž;MZ'?"²±hyX_?ïqº­e~?yϛ•9'?žȯzº-?yϛ•9'?ï¾;;%_?€·l2l/œ?€q;ä€^?€·l2l/œ?ï‡É~tá:?'B
ÛN´ˆ?Ž
 sõ½~?'B
ÛN´ˆ?í·vyY?¢ä—ד€?·*DMC?¢ä—ד€?ì'Ô&Õ¤?›isö—­x?¿FÁ^ÉRß?›isö—­xAGN4FGL J0816.1+4909?íñ[ï·U@@Ü!BoçÀ:·HIÑÛÀ<«¿2°Vu@=>ô‡|@-Ðãe–?À×h‡'üô?°åä Óö?ðbE¥%¾Ö@ùì¿0þ?ïÔ\
G`¿×ËïW;P8¿ãGø½Ÿ¤¿Þƒ.ž#¿ÞNy	×W¿é#7r]®AGNbllNVSS J081609+491005?ïûÿڍ¢?1Ì&[
?@•Zj×?1Ì&[
?ïñ¿¿q¶?Y[Ô=4¸÷?\€';8?Y[Ô=4¸÷?ïòtôô‰)?VΞÂ!û?[¦:}ß?VΞÂ!û?ïÑû"ð?TÖöń²?w9R²?TÖöń²?ïö¾F]m«?EPµQ¦
‡?RƒsªÙV?EPµQ¦
‡?0?nÉÊ)}?~¶(QH4?nÉÊ)}?ïó¸´o'?f1¥HŠA'?YòŽ'¡}<?f1¥HŠA'?ï?•ÎD,?|ÊÖ·Œ?˜MD¬v?|ÊÖ·ŒAGN4FGL J0816.3+5739¿íÔÏH/Í+@@ó¬Äï‰À9'—¾WÀ<1áÜ(Šc@Tåÿù @CrSÍÝ?¥ LâÂé…?¬Ò½–gÐ@¶ÖU⊤@¸õh¢UÖ¿ã~É3»o¿ØG"ÂLÁ¿â±ðrÄB»¿Ý"²œõē¿å¡…¡?*b¿à<	›Š4¢AGNbll3FGL J0816.7+5739SBS 0812+578?ïþs‰@Ë?K¤Ó{?(Ã؁?K¤Ó{?ïô3ׯ?Wfš Ã?Wõ˜¾•a?Wfš Ã?ïô¹À«N?_Úr\%á4?VŒ~oCõ?_Úr\%á4?ïäÿEg_­?X¡+yw…‰?kºÁÛ¢Á?X¡+yw…‰?ïýMN£J?(]õ¨S?5•ŠðÇfž?(]õ¨S?ïЮŸ<­?{T¼¬L?w¨üË.e?{T¼¬L?ïóûˆç£?_&(A=f?X	á;'ù
?_&(A=f?ï¨f¬eé?w°[ééõÉ?…æTßàº?w°[ééõÉAGN4FGL J0816.4-1311¿åÂ¥ëÑ8±@(> ÿT–À8ŸªúêíÀ;Ÿž¾œˆa@èð!Å?ü®»iÍùó?¥xÜI'Í?©Ñyž–Gn@u¦uJ/@ÆÑÜV,²?ï÷$ŸF¬¸¿Ýƒž›3»¿àŽ¡¹"ËÝ¿Ó禆轿àce•†¢¿Ùf=̔CAGNbll3FGL J0816.4-1311PMN J0816-1311?ïþö­ÆÍ.?˜XWµö[? •!uî?˜XWµö[?ïëLló§?qZ­Þ½•˜?dô³L©%?qZ­Þ½•˜?ïç•Ãv6é?tVÚ»¡y?hj<XN·O?tVÚ»¡y?ïúè:UU6?2ía>Uì?D_zÖÿP?2ía>Uì?ïýýôY{?&ƒ',ô;/?0^»"€9?&ƒ',ô;/?ïŠß•ãgÕ?–'"õä×?HygšÐ?–'"õä×?ïßÑ30Pw?yŒI"ƒB?pfn^?yŒI"ƒB?ï÷Íñ(æm?A'h¤qh?Pdfõ€?A'h¤qhAGN4FGL J0816.4-0007¿ïôP7-œN@2Å3	AÈ!À;+÷­K'FÀ<y³J@å´Ð+Ò?ãÚPx¾W¿?ß4þúÇ[õ?ïqèEÏ?úΘ´—Ká@帧ü³Å?ïþÂ^§U¿îPªJè¿Áb]åc¿ËÑexTÐg¿ïÿJ=eç¿ïÿÿ>¹úAGNbcuNVSS J081626-000559?ïØ1Ž‡0¥?q†w¾&"?sç8˅õW?q†w¾&"?ïìK%Ôa'?ejb®M?c´Ú<ø÷?ejb®M?î"HåÖ^?"M>Á­?¦»~ðƳ ?"M>Á­?﷒3Úß?s^n2«(ƒ?'s(±l?s^n2«(ƒ?ï¾p¿
z?†¯³Eîõâ?€cÐ:'µ˜?†¯³Eîõâ?ﵚÍåëF?‰àco }¸?'™L‹¬˜?‰àco }¸?îxË}í@¶?™FG"æœð?¨sH#¿©¢?™FG"æœð?ïÓE³y¥Å?vYÚÐeD"?v]&6™Ï?vYÚÐeD"AGN4FGL J0816.7-2420?è(Ó± ÿó@'ܱF^‰À9މÁµA–À;ÒWF7ò¶@1f]×÷x@Š(ãN'?»a'þ0-V?Æjsç-v0@	¯å†6a@ۉ–AJx?Š‹h(ˆ_`¿áU±wÜ°p¿ç8Ò¿€#¿äi+<Ĭm¿ì~Ø;•Ø¿áâiʀAAGNbcu3FGL J0816.7-2421PMN J0816-2421?ïè.Û÷Z?eÝr«ë"?gÑì«N–?eÝr«ë"?ïàä8p¬2?vS5¿Ñýé?oǞrü?vS5¿Ñýé?ï±q1pa?€(Öp"?ƒ£³ª3¿?€(Öp"?ïõ;¿¯éù?:Ó,p­?Uˆ Ìù?:Ó,p­?︝ˆÞÙ?€LÎôÊÏ?ûX")aà?€LÎôÊÏ?îøäALjV?§ÿ‹"? q»ê]s§?§ÿ‹"?íI¦3¨E?¥¼]§›§ö?³õ²Í†ÖÕ?¥¼]§›§ö?ï¯&:3
?qøòÃES?"6|`'"?qøòÃESAGN4FGL J0816.9+2050?ËSÌ}>@;»ä›«—À:•"¿e=À<f:N°g;@·ëm÷ªF?û<¹t*tH?Â2¡èȀã?È×(ñ:ë@Öoþ•œµ@ãbý%Z-¿â'úÒD?ïû(Êúd¶?'½¨d-ٿӆ÷ µí¿ãð6(°ù2¿ãÂýuâlAGNbll3FGL J0816.5+2049SDSS J081649.78+205106.4?ïݞ%÷‹?sE&1æT¥?q0ö¡â0?sE&1æT¥?ï¿EðF›è?‹ß
¡ãœ?€.ƒôàGï?‹ß
¡ãœ?ïÅÇ^g®)?zÔ-ÂòŠ¢?}P¸;/«?zÔ-ÂòŠ¢?ïaOõ¥wã?rfB0$€«?"ÖSè	"?rfB0$€«?ï¡zFåd?ˆ3»–̇?‡¹¡|è?ˆ3»–̇?ïx;·!{?¤
p¤–?Ðø…¬4£?¤
p¤–?ïš³0TÃ?—³¿=JÁÎ?ŸÌ© ÔŸ ?—³¿=JÁÎ?í€éŸkk?š§HâOž?´ø²(½¬?š§HâOžAGN4FGL J0817.1+1955¿æojŬÙ@;rÍáŸÂ©À;JžWn{ßÀ<£ô¬å¦¸@!±=®6^·?û'êÊä•@?ÏtOȸ–?·ùÓ;PŽ?ꖎý‰X.@Z_Çæ´¿ïù·FRʨ?ïÿü9¡â=¿Òfý:'￶'êΕyÏ¿é2IÉw­·?ÉGŽAAGNbcuCRATES J081705+195836?ïü¹.èÔH?<ðD¤Ž?:6†ž›M?<ðD¤Ž?ïñö¥8^@?_:,3S+?\¶³Þ?_:,3S+?ï¦OQ™G1?†–¶q]ê?†l+™®3Ò?†–¶q]ê?ïéW]›!ë?Qœtδ²'?f¨¢~û¾?Qœtδ²'?ïû"S>ôæ?8Èñô|¸K?Aî²±)Â?8Èñô|¸K?ïÇ«?£?€g vž<?|*kÝ{?€g vž<?hþ¤¿?ŽµèÓÀ;W?—eÎ@<?ŽµèÓÀ;W?戴Üzrk?xór'<'»?…\ÈäÓY?xór'<'»AGN4FGL J0817.8+3243?â'êñÙ@?{y¦µÀ:¯*‰@†À<pê?«ç@ a1R]oó?ý@"Êý¿´?Ï:N°g;x?Èü†c[ïë?ûòˆcp'?ûnºÖ*C ?ïgI}!"¿à–ØŸ8¿Ëñ†ÕòV¿Øx$>x¶ ¿à'¨9p¿éØæZgAGNbll2FGL J0817.9+3238RX J0817.9+3243?ïùVù6V?B!œ±
AÅ?J¤P†-?B!œ±
AÅ?ïÐþ+®Hl?v'£  ó?w€ê@é
Ò?v'£  ó?ïØ÷*Þ?t¡Ç£ÀÂ?sð"ˆÍ…æ?t¡Ç£ÀÂ?ï%ð•g?u»{×<î?›AìPÏ?u»{×<î?ïó	§@À?T1'z§Ã?Y챜±‡?T1'z§Ã?ïÞ?¡\
<Á‹Ø?œ>žvM9D?¡\
<Á‹Ø?ï§ÿÜLOB?†{8ˆò'[?†ß-¿¯?†{8ˆò'[?ì'úÓÎÒ>? Ñ8:…Â4?¾À)a‰n? Ñ8:…Â4AGN4FGL J0817.8-0934?é_ÞEO²@,¥hÍJ¡À9÷І•±À;¾Ñ"Âr@«è¦
?þB>ƒÉM¼?°	ü-7›£?Àñœdûi@/ô÷í@	[wÿ@"?Í 18\<í¿Ø¢°=w/¿Ø8}%Ō¿â<a_–h¿ä|PKߧ¿æ"z~K_zAGNbll3FGL J0817.8-0935TXS 0815-094?ï÷¨íìÏn?N¦N<ނ?P®#§ï"?N¦N<ނ??ä$5?'Ò\õ¤?‹ß°‡VÈ?'Ò\õ¤?ï'tc?Œê䤲°?‹¢ç,;˝?Œê䤲°?ïZô…šÖ?qsô`‹?"½!j%;8?qsô`‹?ï©^]®[ó?‡Ë:¤·G?…¨h—ØŸ?‡Ë:¤·G?ì3ˆé¦ªØ?À½"­n7?¾c¸²Ê©B?À½"­n7?ï-Ò{j?–pR?šE°•1öŠ?–pR?ì_ß0"?œáq›äþ?¿î?œáq›äþAGN4FGL J0818.2+4222¿å/[žtl@@²`˜À7µx!yÍKÀ;lðå°Éa@'ä6>U?ÿïCZD?–µc›þ?µ@j~N¬@ ­¸d"@V{Šæ¿ÄB1¨Ä"Õ¿Ú$¡4˜Ž¿â[Ã?…Q
¿áçø¢=­¿åŠK1Þt¿é3
ƒç€­AGNbll3FGL J0818.2+4223S4 0814+42?ï÷ÉV0õR?ly¢I"·J?PmTÉÌZ?ly¢I"·J?ïÇÁÁg$8?€ôËâø£a?|iJœ?€ôËâø£a?ï±q$—?‰*‹ˆ£–â?ƒ£¶ýÒY!?‰*‹ˆ£–â?ï¼¹t*tH?p Ñd?€Ñ¢êd.?p Ñd?ïïø‡ªrŸ?b«Îƒ
ð?`xˆa&?b«Îƒ
ð?îۛúËì?¶09x?¢FN"ÂÝ8?¶09x?ïËdkJ·ð?ƒ™_ë(©¬?zMÊPU3â?ƒ™_ë(©¬?î΅£\U?š³Qo—:?®Ó¢Zž·?š³Qo—:AGN4FGL J0818.4+2816?î­1ó(gc@>là¨KäÀ:ªp-…DÀ<‡ËCòž@šÞ‡	t?ÿø€¯½È?Æ3©Ðži?Áío"3,?ûÂùå3Ì@5½'"Aç?ïÿqÐ&ôa¿ÔÆÆ"Ž ¿Ç¦F{9‡5¿ç骾…m¿Ó÷V
RÎڿ㟟m1AGNbllGB6 J0818+2813?ïþúk"Á?hu†µN? XAŽw?hu†µN?ïóÚyÀ?Uò"àæíÝ?XK
м0H?Uò"àæíÝ?ïëçÝÒâ?b1&ˆ"Ù"?d"2G·?b1&ˆ"Ù"?ïóXÂd>?;Le¾«Ü?YOÒEDx?;Le¾«Ü?ïýBÃÉîÌ?1ž6ÄX?5é㋆ÐÇ?1ž6ÄX?ïƪGMÍ?"ä¤
ßø'?|ªÜ^þy«?"ä¤
ßø'?ï×w4·94?x^.杰?tDe"Æþ?x^.杰?ïÖò¥ùx?a"Ò¯¼#
?t†­Xf<+?a"Ò¯¼#
AGN4FGL J0818.7+3153¿Ø7ÝÆø«@?vq%Ý	[À;]r{ÛCÀ<´°X"@½ˆÍC•+@‹t"Ì?Ðԍ çìŽ?´˜û(·¯?悬î
46@
½©y
­Ù?î9Xç!â©¿ëL´,j?ڒ1%;ù«¿âg‹_D36¿ã÷÷ˆb9±¿ïÿæ¦SfAGNbllB2 0815+32?ïþ£<8H$?GÆäî5'?%Ì9Ö115?GÆäî5'?ïõ¾Ë­=?Uä+.ž?T'h$T'³?Uä+.ž?ïóªÂ5ïü?^'7ƒ,£U?Xª{.k˜•?^'7ƒ,£U?ïúòÀZZ?/_A'	¡?D4ÿV½6?/_A'	¡?ïÿ‰µBcõ?³ÁIôS?
'¸NÔ?³ÁIôS?ïՙï¢1:?y¾·¦ÃûL?u3AuFÐ?y¾·¦ÃûL?ïõœø|[¤?b³òÚ?TÆd¾î?b³òÚ?ïö:ïÀÜ?DsY`eèµ?SŠ YV¨l?DsY`eèµAGN4FGL J0818.8+3229?ҕœ}f@?žbÜn*€À;.'4ùÀ<b¸®1×@Áœ/ñ	@!"U…?×Â$g¾U;?ÁώÞ§«?ð4Ä}ròf@«Ð9h×Z?ïÀ«÷j/I¿ãÓîÿý{Á¿éq®~-,‰¿à°!/ûpN¿ç&[L
¿ïíp±C‹AGNfsrqRX J0818.9+3227?ï.eQ¤ž—?ÃHYslfä?š3UČõ7?ÃHYslfä?ïóžÀ}g?V;ºy	Â|?XÂÐEW?V;ºy	Â|?ïèTÄ
Ç¥?v÷cæ祠?g«<0R©?v÷cæ祠?ïî‡Ã5ýÆ?C
G<Yä¤?ax<¦FI¿?C
G<Yä¤?ïúÕ(íÎ?GOZÜNbª?D«] ?)r?GOZÜNbª?ïÌÊ<ŒÎ?€"«o]ǎ?yšóöW@Ì?€"«o]ǎ?ï¹W½´´†?…Øo€1è?ª—úH‹?…Øo€1è?ïŸx@áû?uzòж$?ˆ!ïÎ`sÿ?uzòж$AGN4FGL J0819.0+2746?î|LÚ-Í@>j;šàÁvÀ:v[ËرÀ<y¿¼CÎ@‡ފºY?ÿ'è_ÐJ0?ÉIøÜö¼?Ä`EKc¬?ý&ðš1o?þ¿Ý/ñ?ïùï2b¿ä´Ø"óÙ¿ãã9Ü>Z¿×Nø 7­ì¿èLˊ­n¿ïÿÛLÂPrAGNbll3FGL J0818.8+27515C 07.119?ïòÒý,Tá?T>ªÿ(YÝ?ZZI¼'?T>ªÿ(YÝ?ïŒG#)?zÆÌè"Û?~¹Ü`
Ó(?zÆÌè"Û?ïÙheˆß§?oK7Ën4?sKÍV] l?oK7Ën4?îü£ü7ã5?{¡ã8JÔx? 5À?¬?{¡ã8JÔx?ïÜ\ž€M?o†ø'°i½?qÑ°Ñ·tÎ?o†ø'°i½?ïOl¤Ãï? 6šc—Ü?œög÷æ? 6šc—Ü?ïh))øŒ?Ô«•¡?'úÚÀðŠ?Ô«•¡?ëi«S? v:©@£?ÂYS–³"É? v:©@£AGN4FGL J0819.4-0756¿Ô''ÿ¾´@.úò¥µ1À:¸—/\À<igÏòñû@!™9ÍV5?ý?cr–'?ÄG?D8"?ûžû?Íi²KAG?í°T¸'×¥?ï³~è=k›¿é°iS¿å XóÖ&¿Óˆ!Äuæ¿ÖM
ú¿yR¿Ý¹žrAGNbll2FGL J0819.6-0803RX J0819.2-0756?ïü'¡œŒ,?5ºƒ©C§V?;jñU™?5ºƒ©C§V?ïÆüÌòÀ?ƒ~¿Èµ?'?|št[Ñ?ƒ~¿Èµ?'?ïãáÿcøÎ?q(½Î¬?l_Žw?q(½Î¬?懲*<?h¤N±ši?…]9ræ?h¤N±ši?ïû!—]õ?GP½ù"¬?Cy¢E…Æê?GP½ù"¬?îÐAÕýü?¬ Ðhº]ò?¢û❛;B?¬ Ðhº]ò?ïä=†«ù?v\4±Ôù?kÂçgv‹?v\4±Ôù?îb˜6Ô9?—뇄
"˜?®IÖ|'¼t?—뇄
"˜AGN4FGL J0819.4+4035¿ÐºÜ?0—x@@­UÅ.rÚÀ;ZÄ"ðÀ<ÀëóÁ{@ xE×Ћô?þ©Úª!¨?ÌÕ2÷Ï
?±:‰hÉíõ?áDø®ÖÃ@<pŸû2'¿ízÝð,¿âBMb3{Ø¿Þl~Q¿Í¹±<"›¿æ²"L*zþ¿Ý1a¥1'AGNbllGB6 J0819+4037?ïþî$‡ý?T÷Òwå?!±êÒ²Ï?T÷Òwå?ïõÅ÷?UæKo³JÔ?UÄuø"F?UæKo³JÔ?ïóƒ$¸:?k^Ëk'‡?Xù¶"ÊÌ5?k^Ëk'‡?ïøÚ͟
U?1°NjÈ?L"Ê(+0;?1°NjÈ?ïÿÔÂ?=c«õú?åz'Ì%?=c«õú?ïÒ	"Í?w'Á‹'?vû6Zşb?w'Á‹'?ïöý¯1 %?jBÓx¨µ?R¢ °µy?jBÓx¨µ?ïá_ôåÎ.?_É¿
É0?n 1)¶?_É¿
É0AGN4FGL J0820.1-2801¿íöKêAÛJ@ä—t%kÊÀ;nE£x?­À<ŽOËð-û@#'Òëò_?öø¼ßï¿@?Ñúj>ã¸?ɒOù<—`?÷—%¶rî4@á)`Ìt¿ïÿþÐñ?ïþ!xöŒ¿ïÿã_¶Hý?ïÿð`OËð¿ä2M?Mó©?ÁcÄÄÂAGNbcu1RXS J082021.9-280206?ïúº%«5M?A:4b<õý?EhžL(!?A:4b<õý?ïÙ
55l?ÅËÊÅëÅ?szòôƒ'ò?ÅËÊÅëÅ?£x%è?…6Ž	ªï?‡œ×8(?…6Ž	ªï?ïòõ%0'?Q>ñ'V"z?ZµFçѦ?Q>ñ'V"z?ïñïgg©n?[€:î(•2?\!1Tih?[€:î(•2?î–Õ/­þ½?²?ßcß?Ä?¦'­ԑ<?²?ßcß?Ä?ïrãVži¯?"A1'c?'£•%S'?"A1'c?ï­O¯&–?…ÚWT¾º?"¬;aôÊi?…ÚWT¾ºAGN4FGL J0820.3+3639¿îeìzßf¥@@l% Jù#À:,Ú"ö¥
À<uo·HJ@Š%»üE
@"€Þô?¶èô˙q?¤Òhÿ./$?îRœàKß@½½"J¥@¿Ïœ¤ç€'¿áÁ÷Tð¿åùéÀÎfÖ¿áyPFGã¿ånbHÊt-¿ç!ñ¢DõAGNbll3FGL J0820.4+3640MG2 J082018+3640?ïü–bÕ×?,–Ÿd?;Lñ$k´'?,–Ÿd?ïóѶ°E?Wã_O=?YÆ\¨œö¬?Wã_O=?ïø
vúÌÿ?FåwºüK?OÊ$D -?FåwºüK?ïçÓ¶øG?N[³"O?h,èYª?N[³"O?ïøÍh tÌ?A4ò#2È?LÊ^(ª
?A4ò#2È?ïψ˜-£?~ü¾ìâ.o?x;ù¶¨Þ²?~ü¾ìâ.o?ïò<…D?n9 µïœû?[‡óh꽊?n9 µïœû?ï—(Zà?s²¶Ö«DÕ?Š5û°'4(?s²¶Ö«DÕAGN4FGL J0820.9+2353?"ÐñÝ8@=ŸÑx-8GÀ:ÎQ1JüÀ<yôÆ)@¬K&ÄåÎ@l#ú±¦?¼¨ñPdÇU¿²†æ¹‡÷?ô?I)>¾@5."hƒ¿åñ¡mx~¿èOÄÎщ˿äÐà,Ðî¿ã ÷&<ª«¿àWg€桿Λq ?[AGNbllGB6 J0820+2353?ïýh[¼œÜ?(–níòÐ#?4½ «Ð?(–níòÐ#?ïôÓÑ#|?WÝòÀx"à?VYø`x·‰?WÝòÀx"à?ïöÆ%Øq?\ƒá–µÈ?SæsÂ
ŽÛ?\ƒá–µÈ?ïùBºËԐ?2QÍI-7?Jõؽ"°?2QÍI-7?ïö±°šDÃ?I­x_[$?RœŸîYæ?I­x_[$?ïÈG¹Ê]ÿ?ŽÅ£¿J?{Ü#.Ðb?ŽÅ£¿J?ïñ@âÔñ?l?™h´Y?]~;Wä[?l?™h´Y?ïÆJҌ)o?oa½
À(÷?|ږÚ爋?oa½
À(÷AGN4FGL J0820.9-1258¿íGàRÕSÉ@*X©XS~,À:z:iˆYÖÀ<^ߘk¥@֊þÌ#Z@ɀ¤Ö
¾?¿3~݀¤? ÅoôZ?âObcøM?üû@}ž'?ï×.Ož£Å¿àA0íÕ·¿ä%"S·79¿ã%aE•6¿ÝrqÂ:!º¿ïûOyxAGNbll3FGL J0820.9-1258PKS 0818-128?ï÷ÅÙï?BòBÀnÞá?Puô¥æ"n?BòBÀnÞá?ïÝìåq?sråàU?q	TŠC'?sråàU?ïæ;RˆÛS?_ôåf?iÄ­6Œ–?_ôåf?ïÊÄô³"?]_6ŒÓe?z…«µÙÌ?]_6ŒÓe?ïß#–Ýýw?cŸ¼R3?pn4š ,–?cŸ¼R3?ï89²Ĺ? ÄÔ,}ç€?˜øɺOšé? ÄÔ,}ç€?ïŸî|T?~îdh´›:?}#‰ŽÉÜ?~îdh´›:?îéqQžP?‰ßéòèä?¡nèRf	?‰ßéòèäAGN4FGL J0821.1+1007?ï_RÝá@8~»˜Çâ'À:ʺ?+ŽúÀ<‡Q\&M@4êÕeM@…ôäC?ÀxD_U{¿£*RŽîù?â†i`Á¶Ä@
SÉÇߨ¿Þíӄø¿åSŠS«y¿èœ!3Vo¿ß[º9¿ä¢aôçž	¿Ú|=&|AGNbcuSDSS J082054.81+100609.4?ïÿ/"àÞ/?‰ï᱂?*dEQ?‰ï᱂?ïögdWf?V8¾¶W¨?S17D4ÄJ?V8¾¶W¨?ïù)%'	t?9IŸwÅ<?K[j?R?9IŸwÅ<?ïþÃm¹¨?»§àêbA?#É!å"^ñ?»§àêbA?ïÿ-º€?ußÃÏòŠ?zP 	"?ußÃÏòŠ?ïÙ$¸µØX?vÜM÷Ó?sm£³'/¼?vÜM÷Ó?ïøDè<ié?RQc"Øû?Nì^_…×ð?RQc"Øû?ïù)4ã€?=\õO©J?K[/bƒÏ?=\õO©JAGN4FGL J0822.4-2630¿Î:¢™®£}@ãS÷ÎÙÀ;
1'rƒ«À<_")P@0<yûš@uØå	µ?Êúv=Éå?µù…½n¶?îÈ.ØZŸ‰@kk!ŒÏ¿Û½*,ú4?ïïÙAOU©¿ìaÏþ°t§¿ÑHdà
—¿å!){#ŒÍ¿ïÿÐ/WÜ`AGNbcuNVSS J082236-263125?ïüVÁhüª?3æõŠ‹ª³?=Iò¡½ÙÉ?3æõŠ‹ª³?ïÓXxxGö?høtÇ°?vSÃÙ)˜¨?høtÇ°?ïà_¾×k·?gVIŸó†8?o A9h¶?gVIŸó†8?ïêvÖÇM?K,NÀ7º?e‰íÛ[›?K,NÀ7º?ïó'ïÎ{ñ?W$|ûJ?XÜú"þÔ?W$|ûJ?îÙ,vMº?­=êÚ‹?¢m8˜›ïj?­=êÚ‹?ïÆ1¼f?~ü}3?|ç!É;»H?~ü}3?ïo†ºç—?'àž¼Yg?'(¨D÷?'àž¼YgAGN4FGL J0823.1-6330?ͨáñ;À-Y± žÛùÀ;¤öL"'À<¿';ý@"Ùa…«ü?úaAcwž?Òæ">eìC?°=˶¶¶?Ý¡faÞÂC?ý¤¬	ˆ¿Ø¿ïǃý{u¿èó.0D?æ/ùø??¾îê.£ˆ¿é²ò€»|B?Ùã&2ƒAGNbll1RXS J082316.0-632928?ïþ1­ª¦?(WɯOÓ?.|á•J?(WɯOÓ?ïò¢L¤&?_ `€CíK?Z»g"çŸ+?_ `€CíK?ïٞ¾éö?pJv19ÒÂ?s0 ç­­?pJv19ÒÂ?ïôå&#Äð?H¹£kî?V5³MBP¤?H¹£kî?ïþVS'?$"×ofà?*šÑ‰öb?$"×ofà?ïÇlÃTÃ?–hOFOŸÄ?|Iô¤"ê˜?–hOFOŸÄ?ïÒÔMAÏ?{‡D¾ß?v•Ùt¾¬m?{‡D¾ß?ïÜ`´ÜÒ:?k8¯N'´?qÏ¥€h×@?k8¯N'´AGN4FGL J0823.1+4042¿ÐçéçBw|@A
CނØÀ:K _ŠÀ<S½—¥£"@E§håÎ@Ľý&0ì?¸ÛÖÕå$]¿˜Ù·–Ú¢?ßi›"Ö>@KÖWºüì?ê_ëä¿è°Ô^;Ÿ"¿æ†Û†£ó¿çÞavؤ¿ÒB&€IR¿ïü5ۄµAGNfsrq3FGL J0822.9+4041B3 0819+408?ïþ€µ¶Êq?…œÝ.Ã6?'ô¡.»¸©?…œÝ.Ã6?ï÷.þ´ë?QÑlñOK?Qš옩ã?QÑlñOK?ïôW0F!€?Vò®¹áj˜?WQŸÀ´??Vò®¹áj˜?ïÿ[O7?:n!KŸ?ža.­Ã?:n!KŸ?ïþpzUJy?!?"…"Y?(øYØ==?!?"…"Y?ïÙ)Œ–På?tV¦B²÷ ?sk9¿&a?tV¦B²÷ ?ïò*Èç¡ ?`‰Ósõ?[ªnÀ@¼?`‰Ósõ?ïþïQuØ?"eBP0?/养?"eBP0AGN4FGL J0823.3+2224?îÒÇçF@=­gf@¦¹À:q(•J€À<rv.Z†^@yðÿ±üg@#Nƒñ'¨?Á±=òÕ?º"»¼Pí?ö4ƒzsc¥@q,/³ÌÌ?ïªì¨4g¿Æèž9'q¿åèº3mÖ¿å*@ ¯¿ã5ækÚ¿ïÿàŠï²«AGNbllOJ 233?ïû†äÇ?5Åð…Ì?CååøÄ??5Åð…Ì?ïïµß9OÇ?[çæw¦|A?`J ãŒñ,?[çæw¦|A?ïêÙ%aä?\'`¡Ñ?e&ðú:ƒ‰?\'`¡Ñ?ïð¼jÄ?_<§ùC!?~'ùÜâC?_<§ùC!?ïõØ0¥†¯?MÑÿŸŽT7?TOžºr§?MÑÿŸŽT7?ï±u:aG?•áѵL+?ƒ¢±f±A?•áѵL+?ïбb°pÃ?€ÐD¦ .T?w§N½Å`?€ÐD¦ .T?îÛêDŠ|#?‡©5ÓRv?¢A[µ oÓ?‡©5ÓRvAGN4FGL J0823.7-4838?ÎÞé~xÜÀ¤B"ßÎ1À9GÙ.ÚÞÞÀ;-‡É},@'¶iÞì@uò£ +?ÀAž0O‹?±j¿ë½Ô?ñj µ'-l@ÛW‰Ôª'?ëGU^×%ì¿éfA·/'¿è¦¶~¡Ç¿åýÃÝéU¿ìÔ
xÿÆ¿ïù·KAGNbcu3FGL J0823.6-4838PMN J0823-4837?ïò•½RA§?]éÎØn*P?ZԄ׋±À?]éÎØn*P?ïàrä׎?{k*`õºâ?o~:ÄÙ°?{k*`õºâ?ït€÷ÐöA?	jMUè"?'oá¹Íç?	jMUè"?ﴛæ…?hM´
©?'Ù>€ßZŽ?hM´
©?ï½GB×Ž?"Wî쐒?€®/Pl(n?"Wî쐒?ï`Ààd?£áÿAœ¶?"çîGcj?£áÿAœ¶?îmþá`Ç?ŸÂ.¨XÈ?©/ Åډ?ŸÂ.¨XÈ?í‹oêk»?õ|uDÆF?³¤€ªÀ¬?õ|uDÆFAGN4FGL J0824.4+2440¿àŒ.Á"cq@>¢v§&JÀ9žØ:¿¯À<û¶Å#‹@k"+'s@qý"ÕíÞ?°¢"hR#ä¿¢…>©€d?ðÑ}†=œC@!BԐæm?Âcþ"8¿åâX"ÖÅ¿çñâÀÿäý¿áÆýX…Ó¿ç¹û~»òµ¿äGDžkAGNfsrq3FGL J0824.1+2434B2 0821+24?ïþÍ;S8?èRÔe½o?#,M
m-M?èRÔe½o?ïöD2''?Uø:ίé?SwšöxÞ1?Uø:ίé?ïõ8gê8Ý?DݑŠáy?U0‰¥?DݑŠáy?ïÿ­ž£›>ôcñOæŽ?˜[Žã='>ôcñOæŽ?ïÿ'Ý"È?ž"¾Á?bÒ^²?ž"¾Á?ïÖ~‡¢ÿ§?{.z$}õ?tÀ¼"Ôg?{.z$}õ?ïî>ϞŽK?f<ØÄÃç?aÁ0.—}@?f<ØÄÃç?ïÿK`aм?l†.'¸)?"´R?l†.'¸)AGN4FGL J0824.7+5552?Ä­"êžC@AüPHÀ9yú Âî'À<b[ŒÐ×@ŽWáé>@ÀY+",?ªæ%®¨?ž½»"GoM?î\fhå@͘îxîÿ?³ÜÝf"â¿å˜ËЮڿç»ÉÚª"¿èœm¿ ;à¿å(œ×;»˜¿ïÿ±'#áAGNfsrq3FGL J0824.9+5551OJ 535?ïþЄV*H?Èÿvä?"÷·-¿†?Èÿvä?ïöÎ&zNa?Tz™ÕMש?Rc²o¾´?Tz™ÕMש?ïòŒïÅ©?GîaÓü@?[ðåîúN±?GîaÓü@?ïþp^Èô?Ìʍ¬¨?(û|"Ã?Ìʍ¬¨?ïÿ"´Ò|‡?
ÐA<'?Ò×–??
ÐA<'?ïÚYkë?sLnWFo?rÓJv)?sLnWFo?ïð*qJ?`#ð+=ôÂ?_«ÄÞ¦œí?`#ð+=ôÂ?ïüÝÞdq;?0‹2ðŸÙ?9+p®D?0‹2ðŸÙAGN4FGL J0824.9+3915?ï÷®LÕ`@A¦ÊıÀ9'ÛçòÃÀ<Q¶¯T@ü¦–WDà@öƉ¼­?±Ï	¤ïc?º@ÂèÈUð@fhÝ9+›@˜q±CÞ?î¤vlmçd¿ÝM'iÒ,¿ç–ŸV¿äq¦ ¿ç¿ëÙ~áÝU0¿ïÿÏù§÷*AGNfsrq3FGL J0824.9+39164C +39.23?ïû2Då|?6±Éìý9N?C›5ó_úË?6±Éìý9N?ïî¥G!Ҏ?e-íñD?aZ¸é,2E?e-íñD?ïɂª^?|W[* ü?{>õ,Áå?|W[* ü?ﲊ•´v"?k´¯'Öì0?ƒ]Z"'K?k´¯'Öì0?ïò*í&?Tm†KÜ?[«ç÷	5?Tm†KÜ?ïȁ'Öu²?{/&'êù?{¿6‹&?'?{/&'êù?ï|)ME?"¾¡þå?zÖ^;·¡?"¾¡þå?îÔ
ϲ–|?TZi:Ô?¢¿#‹G?TZi:ÔAGN4FGL J0825.8+0309?ÑFàM¡ã.@6c¾˜V£{À9‹¶–ç8À<>æ¾æZ=@쮪ì}@œ@WV?¯_8ÕX7¿@¢>ͨç?'i1qçú?ûA7ë~¾¢?ï7É
ûk¿äÙ¸£J"¿ãœ
!Áñ§¿ágFáúÊ¿ã‹= Êei¿ÙoÐ<ÃÕ­AGNbll3FGL J0826.0+0307PKS 0823+033?ï÷…óýñ»?BèÜ!•Ë£?Pô}kÙÌ?BèÜ!•Ë£?ïîX8âZå?c—CÌ3q?a§Ç$"S=?c—CÌ3q?ïǺ¹ÏÄú?€aàöÊ?|"£LÏ?€aàöÊ?ÕÒÉ«?w…We(Ù?‰ÐŠ',ÍD?w…We(Ù?ïá݈ºVÜ?`cî½0-?n"wPÌP?`cî½0-?_"Œ"E?"ÍÌï4ë??€Ð7NœÚ?"ÍÌï4ë??ï¹ûîg@?"/VkÀ@?¹ý5î?"/VkÀ@?îL?™³~+°Ü?¥Äˆ Ò?™³~+°ÜAGN4FGL J0825.9-3218?ç«P‹]Á§@
tO»)6ZÀ9NW±—½!À;¦€ç,¬@"­K¨@ºZÚA*?·ì
µÂÅ?Ï£Û¼Ô²@è&grÕà@wT©¥€X¿Ù߄ÊÕ{È¿à"b*—ƒ¿éE½úL¿è5QGq¿îÐîdÍ	3¿ëÓb}£™ÎAGNbcu3FGL J0825.8-3217PKS 0823-321?íó–Å»?ɁÀì¼"Ó?°gsJ³)#?ɁÀì¼"Ó?ï½c®ƒ¿?°¯*'Š8?€§PIç{?°¯*'Š8?ï…ƒž@Ù?Ž÷µõ¸?œïOŒ7äÑ?Ž÷µõ¸?ïÕxŽÆà?X±˜_ø÷?uCø3ÍÛ?X±˜_ø÷?íYó×?¸m³ˆiVÂ?µ7ø`k©?¸m³ˆiVÂ?íI|\E'?½X ¬·T?µ´ì{?½X ¬·T?ëàd$Ã?±?8®°?Ãü~o‹lõ?±?8®°?îp˜Ö
?"£›³Ì·?¨ör¢.ʋ?"£›³Ì·AGN4FGL J0825.9-2230?ßO֍ڍ@!ÙöD•[FÀ7ތXhvâÀ;J	{¸@Ô{Aê±?þŽ&žÐ:@?šN‹9•´?°…OŠ¬Á¿@ÿkã}é:@Í+Pæ¢a¿£ãŽZKP¿×ôsúù…è¿á¿6â]¿Û@êa2J¿äšÀá@¿åuÀ –ùVAGNbll3FGL J0825.9-2230PKS 0823-223?ïû®;‰Y?<‹.àÂ)J?AGû¤¨(?<‹.àÂ)J?ïÙÔû£«?'zè"ѨZ?s'âÂÀ?'zè"ѨZ?ïã^µ©*í?rèݞ#-?l¡Jy1*?rèݞ#-?ïùû@þwë?2çüÂ/4ê?Hü!5e?2çüÂ/4ê?ïüFìãe?5â˕êp?=Ȟ"S	<?5â˕êp?îºÒÀÆs?¯¦ìz}yÇ?¤RÓõP©?¯¦ìz}yÇ?ïä êÀ?|KŽ2ƒ?kßêì'?|KŽ2ƒ?ïî{xؗ?QŒ<é·M?a"‡°®I,?QŒ<é·MAGN4FGL J0826.4-6404¿Üó-äê¥ÑÀ-XçW'Ž
À:‡‡H^>À<='JSá@!ã~êì?üqšânõ?·SÈ)$?œ(b}VK?叀[@áäÃ
±D?ëEKß&–˜¿àȳÞq!¿Ò•½Áìõ¿ßû[O¿Ø¡ŸAÏ-O¿ÌŽ9G¡AGNbll3FGL J0826.3-6400SUMSS J082627-640414?ïþ«|Eð?^ƒl¯?%H;"8ø%?^ƒl¯?ïôd¶ñ?[¬½j«è?W6'sjœà?[¬½j«è?ïø4¤ÍT\?V17":¥?O-lž&Òæ?V17":¥?ïø'¦l¼?7$dÇSˆã?M»Ý@^.?7$dÇSˆã?ïûõÿB;?8Aèû¨·?@(ÚÚò&?8Aèû¨·?ïÐ4§7Î	?–jºƒÖ+?wå¬HœÂ?–jºƒÖ+?ïö
ÃÓSú?dÄKFîÞ?SêxzTJÖ?dÄKFîÞ?ïïZ$}|œ?PKSŒå«?`¥ÛZ§ëë?PKSŒå«AGN4FGL J0827.0-0708¿'}6F	Ã@1† yKÀ:¼gú»À<5m%H{@ ®TL2ˆ"?ú݁5ž?À1xÞc"9?Ãúr¢^å@7ßÖjÛ@ûEá`­•?ïòMZ%æD?Ýêßqêþç¿ÂÑå:Ü¿Ï÷ ÞFò®¿ã™:Ü¿ÖElÜ!SAGNbll3FGL J0827.2-0711PMN J0827-0708?ïû_"qÿ?@äy©É™?BïZZ>ù?@äy©É™?ïâ¢X<?nªÅÕþtô?mê^"{x?nªÅÕþtô?ïêË]QŒ?gõ"§m&?e4듐+ä?gõ"§m&?杻˜s?fõÂÖ|?†ÙÜ_#í?fõÂÖ|?ïòLi¡?'?TŒÉžçX·?[g,Ó~\ô?TŒÉžçX·?ï&!ÁŠ"?—ïä?_Zf?¶w[4?—ïä?_Zf?ᅲÃç²?z4©žØ?€!ÿ‡?z4©žØ?îý¨dž9?‰¤sÐ!å? %y¹¹Ñq?‰¤sÐ!åAGN4FGL J0827.6-3735?àrOßÚ?áß®PàÃÀ9\‰Õ×7ŠÀ;-«‰†&@ŒhF]0@ì["e…–?Ì,Ë:%•¼?Îñ¬€&+
@%[Új@
±´Ãk¥¿Á«w½{Ëþ¿å`=Wyc™¿ìD‡•¿ïýÜ¿‰k?âɃ¡àø¿ï¶1J$ç@AGNbcu1FGL J0827.9-3738PKS B0826-373?ïÜ3Ýÿ¶?ª©_rFès?qæwô#m?ª©_rFès?ïßU Ôòò?†ve<8Î$?pUo·ë?†ve<8Î$?î1BýÝÞ?ŸïÛé?¬ëßÀþ	?ŸïÛé?ïÿz€ñúP?
lb¹N·Ÿ?¯ÝõŸFO?
lb¹N·Ÿ?ïíЮêÊË?v\ßsª\	?b/QT½*?v\ßsª\	?î¨Mó9.[?²¿ååãÏ<?¥{ ˑ3P?²¿ååãÏ<?ì4åÞÒÄð?¬`§FÁµ‹?¾XÑ	i؃?¬`§FÁµ‹?ïóÆÀ:»?ZP¹r|E2?Yðr"+q?ZP¹r|E2AGN4FGL J0827.8+5221¿ïÑËup@AÔîàóË>À;Sx›ó-À<¸[j‰á–@ ‡%["5.@µPy•T?̊›9ÖÚ¿Í¶ùôº?Àvþ#±àã@¿ñÇx?ëKå±  œ¿è	cr– ¿è]ÕÉ ¿Úm¾I|K¿ß[ÿDÄ*<¿à]¾÷÷ôAGNfsrq3FGL J0828.5+5217TXS 0824+524?ïÊn@ØëÈ?´
p%¿È¦?zÈß|,ÄU?´
p%¿È¦?ïõªtcÍ?T´€t?T«¤A'e?T´€t?ïðÅ+e+?pxZ‹8@?_ÖuÇr9í?pxZ‹8@?ïø&E¾?1jÞwÁÎ?Ofê»ï
€?1jÞwÁÎ?ïþ¡jb?NÛÀðO?&.*#E=?NÛÀðO?ïÑ+ å	Ò?{Ϛóæ?wj/umÓ3?{Ϛóæ?ïòò'.?su¨ßkæ?Z±~î²?su¨ßkæ?ï×þü§?c#ɊÚX`?tž%l"?c#ɊÚX`AGN4FGL J0828.0+2307?ï×z()@>ﯷéÀ;
ê0ŠâGÀ<Ÿ	"5"@ ü¢¥‹•?üÉJç"Þ÷?Çö·ÂN™–?¸'ˆá±O?ñØyÞé/@~ç­Î¯Ñ¿™ª8€Ø‹%?í¨ÊߌÂò¿Ø•Þ#6eî¿âHdóŸŸm¿ÉÞ¶Ö:µ¿ê³
¹—eãAGNbllNVSS J082801+231215?ïýÍoMÚm?!«-ý8;ù?1"…ENÐB?!«-ý8;ù?ïïžr`3‹?]ˆhEðïQ?`a©k\¼?]ˆhEðïQ?ïîòÿ3ã?_ƒ¶$2?a
øñ­Ô§?_ƒ¶$2?ïà›¬vô‡?SâXSæ?odSxYi?SâXSæ?ïü"¼×{?2‡_~¦?;ÚO&Ò?2‡_~¦?ïºêžç-Ã?'=4SBÁ÷?EXHœI?'=4SBÁ÷?ïíöD.Fÿ?m:øAwF?b	¼ó±?m:øAwF?ïxÈ.5%.?€O"œöè?æú7£Œ5?€O"œöèAGN4FGL J0828.3+4152¿ï÷fÆ|7@A˜©Þ‹;2À;›ík¨Å‡À<â{s=å>@!6ÛìOt?ýÖ`)5ƒp?ÍW³›"…¼?˜';½'v?Ιë£ýu·?úYC[öÌ¿é|O÷Æ¿îEÌþJô?Çg_	й@¿é&b@¼ß¿¬ÖI"]Í濸%^^Z(kAGNbllB3 0824+420?ïÿ'3[Þ3?=öþñK?"5ù/?=öþñK?ïô_­‡?X{ü`S?WÉ÷SâÁÞ?X{ü`S?ïåb]]??kœ
?j¢Ø$¡L?kœ
?ïùðH€Þ?6Xn|ÏW?H?ƒœ|L?6Xn|ÏW?ïþ°ÆB*X?!<–Zá'A?$ó $w'?!<–Zá'A?ïÑ1ªX±?vEwRgA?wg*çvOŸ?vEwRgA?ïèýŽ¥c–?nHf°ìý?gqp™éË?nHf°ìý?ïÙ SáÃC?m}>2Ui?s/Õó¡~¿?m}>2UiAGN4FGL J0828.6-0747?æ*ͳýs@1‡"%RDÀ:›ÇqC9À<l_˜ìËp@'ÖÃñ†ë@;™ÔQüL?ÔÖàâXz@?ä–ëip@µV=ú6'@èHÎÐÝþ?ïåÃ=×Ñä?>ê!¿ëÃÏ,ù]O¿âËñqÇÿå;Ðá.ƒ¡¿åIßG"ÔAGNbcuNVSS J082854-074854?ïðOÐÅ!T?ayºµT×d?_`^ˆH&?ayºµT×d?ïZe«,?›kÂoƒÏ?"³^#½B˜?›kÂoƒÏ?ï?áöïNò?Šß'S³¸?˜Á(õYÃ?Šß'S³¸?î»ÝãdW²?ˆÀÁ-u?¤B!ÈޝÞ?ˆÀÁ-u?ï·Í'˜Ä2?ŽJøÂaƒ?'›Ÿþ??ŽJøÂaƒ?ëáåŸùÒa?Äi,ÔÊG6?Àxi€¶}?Äi,ÔÊG6?íå^iW?¢žÌäh­?°×Õº¨Ë?¢žÌäh­?æóa("¼?·crœ"â?Ò=ͯº‡?·crœ"âAGN4FGL J0828.7-2422?å4ît<h@ ÀîIõ˜À:̹-³—rÀ<\w—|@^Ù<å@
¥³Ú?Å¢7"0?šP¥<˜•@?Ö¡ô›<@f
#‹?ïÿ€³ï†5¿ç¼"¦Ò¿æ"
q¿Öž:}ªOÊ¿åïŽÎd|¿ïÿz)5ÙAGNbll3FGL J0828.8-2420NVSS J082841-241850?ïûûe³Û\?F¼$À÷ÿó?@iºð ?F¼$À÷ÿó?ï喨§?xŒÕë "?jiWb¡%?xŒÕë "?ïëížáW?m`҇Zª?dÿ‡šH­?m`҇Zª?ïòÃ0cA?<kŒFk?ZyŸÂí>Ì?<kŒFk?ïüù÷ìúÙ?5]±*Çì?80A=sÐ?5]±*Çì?ïW¼Uÿ?¢|å€cB?•u^?À#?¢|å€cB?ïçËáóÙ	?sD…ZKê?h4ϭ׆?sD…ZKê?ïÆU§§N?e¤yf>À?|õU'\äÕ?e¤yf>ÀAGN4FGL J0829.0+1755?é¢Eàl<@=]Ù©T"À:pÓ¥¸À<t3Øt ¼@¸ÂÒ¢ú–@7·&rZ?Á=¦©¢{?¹õeó#ù"?úo|—@‡sÐÝ'¹?ïä"pB]¿Ü•)<ºEŒ¿ãðís5Â¿ÞŒ~þã ¿ê†-vZÐ0?™BüÔÒTÌAGNbllTXS 0826+180?ïõYê	Ò?U"‡¤`/?UL,VÌâ?U"‡¤`/?ïî$`åü|?^XoÎ\(|?a۟'Áó§?^XoÎ\(|?ïÒè®me?|E­hîRò?v‹©è5U?|E­hîRò?フž+)?`Oƒ½cŸ?€\Ø$Ñ°?`Oƒ½cŸ?ïØ7e¶¬ê?r—
÷Át?säM
£??r—
÷Át?ﺐw\	?ƒv"ö3J?[â(§‡¥?ƒv"ö3J?ït"…FŒ"?BJ‰X\L?'ooUvŸ²?BJ‰X\L?îÌö›ÛÆÃ?†Jþ–Ê'?£0–CzÊ?†Jþ–Ê'AGN4FGL J0829.4+0857¿æýÖzJžà@9ÐÉûa4ÎÀ:ΖãܳËÀ<'ñŒŸ¶@6"1Rˆc@‰ek"¤?Á€¸HÜ=¿] "øáL?WP¸˜ý@PeAxEa?ïõ+Z÷[¿âH^=¢ø¾¿àÖCnÙÒ¿á`{jÚin¿ßò)é•ö¿ÕwyÿJxtAGNfsrq3FGL J0829.3+0901TXS 0826+091?ïüRlù?/fïf±??n3nð§?/fïf±?ïôà÷?U¦Ì¨ÿ®ò?V?óµ—Ő?U¦Ì¨ÿ®ò?ïóǏ˜†A?VèG_¹›¼?Xpá-Ž†?VèG_¹›¼?ïô ;êŠ?9ׇ6õ?W¿‰î*ëf?9ׇ6õ?ïù»–!G¬?Ac˜m%?I¨~]hv?Ac˜m%?ï˞`Ë\?"ìM¢s~?z0ϝåî,?"ìM¢s~?ïóBðóü?iRx6<é?YzùË=˜?iRx6<é?ïÕ}‰ÝRÆ?^$+s˜H?uA;·µ1?^$+s˜HAGN4FGL J0829.6-1140¿íüúíÐD@/T)¥ë·À9ÍRúxׂÀ<9KWí&ß@Åq%\0?ÿÖeÒ°?µ–È®ÚôX?²†8—·?ýÄxœÉÐ@K¬Ñ¯µ?ïÿÿÊPË¿ß±$ûŒÿ¿ãì@§Ú¿Ó¯ÎD¬¿ã‰u_'®¿éÚ~Q1AGNbcu3FGL J0829.6-1137NVSS J082939-114103?ïü°9ež¸?0ð©DLé?:~5'öAt?0ð©DLé?ïê1ÄjŸþ?gÍD7°¥?eÎ;ظYH?gÍD7°¥?ïðqf8‡ö?k Ïª`ú?_3Þ§Y?k Ïª`ú?ïÓ9P·06?Y
þ<®â?vcW«Gó?Y
þ<®â?ïû¥'°ôÕ?<[ "í?AiõWBŸ?<[ "í?ïœA		¾ñ?Ž-¥X?ˆï½½CÚ?Ž-¥X?ïåõ•måâ?usÆ{Åã??j
jP!žÀ?usÆ{Åã??ïi9e–!?vþ¸ª‰2?'ÜXÖ¼×æ?vþ¸ª‰2AGN4FGL J0829.7+5105¿ÐÏgÖAÚZ@Aûd­ÿ',À;A³àl½À<ÛãÛÝ@˜¥ûý'ç?ÿµA*l»?ÎK`æõ—ò?¬øƒcø"?á!aRüQ?ûZÈΪ¿æv!ÅL¥Ë¿à…'âr%Œ¿ä¡‡¿}¿ªcÃ|t£¿ïÿ"Àh¡?ïóÕðaýKAGNbllGB6 J0829+5108?ï÷Û6?F"Íõ¦Ž?PIÊ54öM?F"Íõ¦Ž?ïñ~_=?XùLö?]Ö úö¨?XùLö?ï¤çÁ6?Ñ;<Þ*?†Æ>'€Þq?Ñ;<Þ*?ïæBAn	s?VýéYT.?i½¾Ë¯ü¿?VýéYT.?ïú4˜§Åñ?HâF×Êz?G-
X"Ý?HâF×Êz?ï°3Lï®	?…™ª-:¡?ƒó,Êóµ˜?…™ª-:¡?ï³äÉ÷8?†§1Î'l‹?ƒ̓éʃ?†§1Î'l‹?ïW5òçNê?‰º¾ù ?•A¡^T·?‰º¾ù AGN4FGL J0829.7-5856¿áÜ·jSËÀ'÷¾æÀ9Œòã·ÊÝÀ<<ʋ©í@J€×¬@€Á@§ü?µØáò½'?³HÐ(ví?ûˆ5©/8Ó@éI&÷ç¿ÔI":<'¿å§zޢ߿çÖj¥Gá¿æ¯qr3#C¿ð?ïÆ1bM§ÿAGNbcu3FGL J0830.3-5855PMN J0829-5856?ïšü‰d(…?©Øx&­=æ?‰@ݦõÞÐ?©Øx&­=æ?ïñ
í}û?]v
íE?]ëø%
@?]v
íE?Vyðm?ˆ3õžÿ¿P?Š'jZ¤¬Á?ˆ3õžÿ¿P?ïäeaG‡m?Y³œµçݼ?kšž—|SN?Y³œµçݼ?ïÞª*
•…?vaƒ'j?pªêà˜5ˆ?vaƒ'j?ï«]lÓÏ?¨xÄ1Ô¬?…(¤À½jœ?¨xÄ1Ô¬?ï^RÔî?˜O¯"÷†C?ž45¼¥bP?˜O¯"÷†C?îìBB§Þ?"œJ$ƛÌ?¡;Ûá-P?"œJ$ƛÌAGN4FGL J0830.0+5231¿ìœ·…+½7@Aÿz¢]zÀ;ðG%XÀ<¼•¹:I@ žBFK"?ÿƺ~ìo*?Ι>ív?~r‡î¿?ªDOÿáeû@ÍãùI¿å -à
¿ÜÜ
œö›R?îÞ!¯é¿ßu¸ÿ:ˆ<¿ìwÛ~kjÝ?ÛF.b"óèAGNbcuRX J0830.1+5230?ïúéðôõ5?CŒ@%A%?DX<s£Å?CŒ@%A%?ïõStyØ?X[m™Õ'?UYrMÆ?X[m™Õ'?ï'Ú
?'ÒÀ¬Uýn?‹¼	z
Ð?'ÒÀ¬Uýn?ïí&¯ŸÈæ?VT)ë¾V÷?bÙP3Y'?VT)ë¾V÷?ïü•¶ÏÏ%?3 =vI?;RHKw?3 =vI?ï×~s«ý?vqÇSÍBÐ?tq@¦™Ã?vqÇSÍBÐ?«Vì‡?‹1õ<úԔ?Ž4"².?‹1õ<úԔ?ïÚNϊ±
?oØw"ýÈ?rؘIÕK?oØw"ýÈAGN4FGL J0830.1-0946?ص™Öf½@0ÊFà!qÀ;A8"ÀõÀ<©!6±m@ ìcÎ[˜,?ý°áxÚ?Ìh´‰ßè3?£ý?[_¢'?Ü:…M\T@?%ƒr:Û?ïÿùSt¿èýÒ~<›è¿ßŠ'¥aMù¿â9gàd`¿©¶I¨•Šì¿àÚ¡'µ AGNbcu1RXS J083014.6-094455?ïÿwØ1b?^n¢Ø¤‹?÷§Æ0?^n¢Ø¤‹?ïòà©އ?Z
4º%	?Z>­ëƒAÏ?Z
4º%	?ï÷TIG5?Uk2Ww?QWm*…?Uk2Ww?ïþûðC?gì¯ûÓ? CÂP3?gì¯ûÓ?ïÿ¿"Ôb>û?o:ï?ÁϾ–è>û?o:ï?ï¾çð×¢?†aåLš·?€F<÷Ãuª?†aåLš·?ïøˆ™ÆÌ?["M¿Éז?Mßµz'f?["M¿Éז?ïüOIœß¨?2Ú0Ëå•k?=…´>""(?2Ú0Ëå•kAGN4FGL J0830.8+2410?à_>±ºo@?ÛøvžÂÎÀ8´wcä¬À;܋Hþƒ@ÿ).L™Œ@L±:?¦SN† Ã"?À³Eý9@ù/+f¶@—Šh"¿×ÔÁû¿ã9[e¿æà›$´¿é:귙^á¿ì½Ú@¨¼¢¿ïÿïXzAGNFSRQ3FGL J0830.7+2408S3 0827+24?ïòœÇbb?Y
IŒ"Z;?ZÆq÷8»?Y
IŒ"Z;?ïòžR»ä?c/ì)z÷ê?ZÃZV¼eÿ?c/ì)z÷ê?ï¯R{Lý_?€Ÿ‰,ˆ?"+a'™>X?€Ÿ‰,ˆ?ïÿ'B÷?<$›ü?ojYbHÆ?<$›ü?ïò+oU´y?S²áѪ¤?[©!ÛG½ò?S²áѪ¤?ïÏéŠÎî?{a@ð\µ=?x:Ï<qS?{a@ð\µ=?ï¾%΁éá?…n†6Q"?€vŒ]͹Ò?…n†6Q"?ïþæjá(?TÞõ
Nu?!™Q}Yz€?TÞõ
NuAGN4FGL J0831.4+2631¿ì-'Åjü@@ZŒÞ 3èÀ:یwr'eÀ<r7€ŸÍ@í5eèg2@+Iº?Ê°9FÅ?¢ô¤­Ï?Öin¼ó¼@ëpõ3s¿ãà]¾!8_¿áË¿¹Ó¿ê'Úgê¿ÞØ|ßy£¿ïýĆ­-Ë¿îÍ´Þïd&AGNbcu3FGL J0830.8+2629MG2 J083121+2629?ïûT¤òé?:RR	9Á6?B­luÇj?:RR	9Á6?ïógÌu—?X'÷Őļ?Y0f¿š'¿?X'÷Őļ?ïß?k$ç?eÐ[m©µ?p`Jv{qb?eÐ[m©µ?ïð9cxö6?F9sô×ç?_9)sà?F9sô×ç?ïù‰hkp´?GAÝÓ©Ñ?IÚ^@¥—"?GAÝÓ©Ñ?ïВ¡z0?vOBËf!E?w¶¯.JMþ?vOBËf!E?ïËÿ'‰ïq?}Cûi¯§f?z7PUÛ7?}Cûi¯§f?ïœE=ÕV?x¤'T<I0?ˆø®©«r{?x¤'T<I0AGN4FGL J0831.5+1747?îÿÈï·L@=Úþ£ßm¹À:µq5ÍÀ<~ùÛ"Ðå@ ¤ßðbÿ?ü2ÑɋϬ?È	¤"ZS?ÈBY@ãö@¡³CŽË	@?Ücï(
u¤ÇË?ïãՂS?ǒ£Ì´ú¿ÝiÀ8î¿Ýïø€¯½È¿æ«œ 1£¼AGNbllGB6 J0831+1746?ïþø~×L?$Nµœ@²?.PwÎ_Õ?$Nµœ@²?ïòDZøÊ?V̇Ú3Ѓ?[wIß±NÂ?V̇Ú3Ѓ?ïéAªšGê?pµ³j¢ù{?f¾U@œMä?pµ³j¢ù{?ïß߆]Õ?T+ëϝß?p=.mU?T+ëϝß?ïûIc›·?@u)«æ=?BÚsЭÉ?@u)«æ=?ïÇËÓþo\?{¸µÁº?|ùéò?{¸µÁº?ïÎɲn°@?Ð&Ã	?x›&ÙÕì(?Ð&Ã	?ï¡õ,V9?t¬ÙOÚ?‡'´ÙC±8?t¬ÙOÚAGN4FGL J0831.8+0429?æzf©_èÑ@8YVŸIÀ8,vü¶ŸdÀ;«UãTÏ@yïJ%=&@rN¨Ú?-ÞM?³{1yŸ©(@ÃÉîËû@;ț9×½¿È••~Å¿ß4ä"ÔÁ8¿å$ŽTÁù¿ãŸLa¢—¿èþ5$¤û¿éáä¡ÂAGNbll3FGL J0831.9+0430PKS 0829+046?ïûë³?;NôÓ{»?@S¶ï?;NôÓ{»?ïí¬!AÕI?sxa!@_?bSÞʉOA?sxa!@_?ï脜:{?j©TJ£ð?g{c…VÝ°?j©TJ£ð?ïý}t¨|?#$ mÓ(?4\7tD¥?#$ mÓ(?ïþ.LïÐ?'bá2Ÿ¹?-
¯DíŽ?'bá2Ÿ¹?︙CÞQ/?‹Ã¬¸fV?Ù¯ú\?‹Ã¬¸fV?ïðˆ^fp?iºÖÐ譁?^üïùž?iºÖÐ譁?ïøÕ°1qÎ?A"ÝD?L©>6¼®ü?A"ÝDAGN4FGL J0832.2+2753?ÚÆp8"…@@ ì•¿ðEÀ;8^B«v;À<¨PŸTÄ}@"Ô¿Šo@'™Ù;?П‹€Ò"w?¿_ë^C"d?ìv¥CÃ?ø3 Ä̊?ïñ`®–¿äë‰>ÿàK08¬ð¿å՟¿MˆI¿êg+R"!‹¿¶‡ä‰ŠÙAGNbcuOJ 250?ïé¸ø¦ç­?š¹¹
—0?fGpuªš?š¹¹
—0?ïÈ-ǟ¢ƒ?€ ÛÜüò?{é!zr?€ ÛÜüò?ï¢
?㴊?†cOÍÌ?‡}p£Aœ?†cOÍÌ?ïyO¾‰`?p"MTe•®?Ö?&¡ù?p"MTe•®?ïÚ¾lâ¬]?pÝ$Fzõ?r É£÷eX?pÝ$Fzõ?î×AçšÈ2?¤  /@!"?¢‹áƒ¿Çé?¤  /@!"?ïpbêj9?ŠÞs4ºy?'ó½[Ӏê?ŠÞs4ºy?ìŠGÖš?¡ÆØäT ?»­Ç	O›/?¡ÆØäT AGN4FGL J0832.4+4912?ì݉èe@B1yЦv!À:A0«™v^À<˜Ç¤nß²@¾]r¡Þ@¾\ǁ3?µõÞ;¿ŠS‡;žÍ?ԘÂÚô?÷÷/™Ë˜š¿ßÞ¿þÞ÷¿ãc-ÌÁå¿æ®x?'æ¿ãU1Š¼‡¿å%yœÝò¿äF="†AGNbll3FGL J0832.6+4914OJ 448?ïùå!'a?@j‹]àÚ?Hk{ˆ)Ò¡?@j‹]àÚ?ïç螥?t¥™Ô;Nà?hýýž?t¥™Ô;Nà?ïΪð®ÿ1?{S÷јƃ?xª‡£°óJ?{S÷јƃ?ï§Ôüi?p'Z`–g9?†>¼Cá­å?p'Z`–g9?ïïÖäË°?UYY
R¥?`)(Ž¸??UYY
R¥?"+Q¤?•4ý	ké§?ŽÛ.L_"?•4ý	ké§?ïª&¤ùR?†ÂÌ»&~'?…vŒrם?†ÂÌ»&~'?íÈ*j{¯?œî
ùÇñ`?±¾¬¬ÿy‰?œî
ùÇñ`AGN4FGL J0833.4-0458¿ìÏÉVu®@4+"Ù@yÀ;çÌ,"ÝÀ<èj±NÂ@¦9$¹È¹?ú6çÚ+?Ôö+ÀÎð?åÞN4@ym@››]@'~ã	û?ﮔ"6`º?ְߛÜiù? +€À"À¿àvH¿ïÿ­?å`¿È~£®$kAGNfsrqPMN J0833-0454?䒱>ë'ù?ËÓdª'(?Öڝ'(Ü?ËÓdª'(?ê*ß@ff?ėäÖ·dä?ÇTñ'þfg?ėäÖ·dä?â¹f܋H?³[ÒNA¦?ڍ2Fèáo?³[ÒNA¦?ë=*Æ©?¡ÊÖƒL)?ÃUË°å]?¡ÊÖƒL)?Õæºþ²ç¸?Éý§MÈ¥?å¢€¦Œ$?Éý§MÈ¥?×N7i}1?Ñx¹'˪l?äXäKÁg?Ñx¹'˪l?ÍõëÛl"?´¶Ð_âk?肅	$ý÷?´¶Ð_âk?á˜.Ãj?»ò×£j~?ÜÏ¢y*ýô?»ò×£j~MIXED4FGL J0833.9+4223¿ì»2Ôú©æ@B"ÂÎFIÀ9Û‡\€4À<uJïèZÈ@#S—+Ö@<A<
rJ?³ìhžyþ?¥z{TDP?ðœí¬@eK@
U€ºûi?ïþ,‹yEf¿âϕ¿ol¿ç'K³žÓ¿àmš7NJç¿í§VPn­]¿ïñÍ!ÜHÁAGNfsrq3FGL J0834.1+4223OJ 451?ïûCN£?7$q´Æ
?BòÅßloC?7$q´Æ
?ïóÇö#]R?WŸJUäæ?XpqÍ{â?WŸJUäæ?ïÏ`1\Þ?{j0aÓ?xOçö́¹?{j0aÓ?ïÛiI^‡?`ª
ºu¯?rK[FmdÂ?`ª
ºu¯?ïù;E<?A"%x³u=?K'÷…5?A"%x³u=?ïؐó¶N9?uñ:¢Å?s·†4§'?uñ:¢Å?ïÌóY4*?
w]ª¡?y†Sq7>÷?
w]ª¡?Ñ[Qà?vñ¹%Û?ˆ_¬›#é?vñ¹%ÛAGN4FGL J0834.6+4402?é\?j'ß°@BFK†ýÀ:yÞfRDÀ<§—L¸?w@Ý(bŸ²b@CF uÁM?¿iS֖Ð?½§Žú¯34?üK‡mG+8@	E…a~J3?ﭓK¡¿¿s?|0–åy¿äO›HÆBo¿ãð`̞¿á²¬ÅÆHN¿ïü:]Éß³AGNbll3FGL J0834.7+4403B3 0831+442?ïþ·_Á? Ž—r]‰:?.ԍ	#"Ç? Ž—r]‰:?ïô6£€"O?VÒlýT5?W'¹~-æ?VÒlýT5?ïð>n¥¥?bÛm¹ä?_ƒ#ª"/?bÛm¹ä?ïé2ɝ‡?Joi9ÒÆ?fÍþ5 Ù?Joi9ÒÆ?ïüz‡ä!?5¬åÓ»GÏ?<+¿lµêI?5¬åÓ»GÏ?ïÓ+A†'?uÃ•'¸"?vj~h+³›?uÃ•'¸"?ïìæŽÀ?mßE³¯?cîµøt?mßE³¯?ﳓY¨V»?kŠzåÊÚº?ƒ)¢ ßJ?kŠzåÊÚºAGN4FGL J0835.0+6243¿ìÁŘâ @AÙGNΚÀ:ê"@lÚÀ<ˆ$GÝå#@SÒ¾SbS@<=3g6?øŠØ¡e?¬À'¤)añ?Ø9ºáè¾?úu…•Ö–z?ïþÛ½«q³¿èÝ¡ÜF¿ífÒ1›Ä¿êŸ—£ö¿ïJ˜ñÓí¿ÞÃÓߐžÉAGNbcuGB6 J0834+6249?ïYæ*Áʐ?¼"¾¼ÏåÂ?"Ã:§Æ­ú?¼"¾¼ÏåÂ?ïIT"¤3É?§ß'EºÖG?–ÕmfRí?§ß'EºÖG?î.C½Í‰?¡Ãå55`?®íÂkYq?¡Ãå55`?ÇUG8?€¾q pç2?ŽŽ1j?€¾q pç2?ïäæFùí?zŽí¼Ô?k¹4͐º?zŽí¼Ô?ê]ˆWŽ?Ì>ÜGÐõ?Çâ‰Þ¡Ç¢?Ì>ÜGÐõ?î´î Bfh?œí1­]W?¤±ùEä?œí1­]W?èXlú:i?Át™\)n?ΞL\?Át™\)nAGN4FGL J0835.2-2243?íå_â¤â@%›™N?À;>ŒjÜí¬À<߄ۜsi@@'I}"@	ۛœ©?Ö £ylS?ïÿülò@ÿ3å	Út?ÿ4]q +?ïñô¿Zƒ¿á½Zi¿àøú'0?¿íÔ-ê¿ïîÌț¿ííËJÍÈAGNfsrqPMN J0834-2241?Ûõu‡…e?ÒÎÒ$i[?âE<}½N?ÒÎÒ$i[?ÛìFî/?ÌPÇ~ëT?âq	܈é?ÌPÇ~ëT?è"0èÄéÃ?±¹³Ã›´?ͯ<\ìXó?±¹³Ã›´?×
w°Ä6?²-4ó¾y?äxzÄ'å?²-4ó¾y?Ößé2Ò?Ѭí}‹4ì?äpf÷—?Ѭí}‹4ì?­…DNh?¹þwÃÀ?î'¯ëÚGù?¹þwÃÀ?Öü )¶?»2'¯Ù]:?äïëy¤ö?»2'¯Ù]:?¡'\°íä™?Žâdœ^[Z?îçÚ4Çæg?Žâdœ^[Z	MIXED4FGL J0835.7+0936¿é T5ƒ¼Û@;"È6eÛÀ:ÛÉÃ-ÚÀ<Š€Þ·°Ü@Êõ7O!¦@·{¿"ÿ&?ȂÛgj?¦"¶]Ÿ˜?ã—ñ=Å]m@ ÄÃéÏ<?ïûB0&8¿Á%l5³@4¿ç¾"7Z	¿ß@\[˂˿ål¯UÀô¿àÍÛÀ…—AGNbll3FGL J0835.4+0930GB6 J0835+0936?ïþÀ–ÍPD?¨,ìý?#öŽüÊ?¨,ìý?ïôId?X'$Yx?VåòëËç´?X'$Yx?ïõò'¥5"?V¡bñ%±?T°‰™ø?V¡bñ%±?ï÷ZTÎþ?1Ý^4|?QáJë.4b?1Ý^4|?ïýµZóÊ?,5¡Æ[¶?2U)"Y8à?,5¡Æ[¶?ïÓðq[{Á?yýx[Dk?vÇP2[Á?yýx[Dk?ïùæÒÌ/?O‡u7ä¶?Hdµc&F°?O‡u7ä¶?ïݼXWÒF?X¶OÒ
,^?q!Ó»Y¬÷?X¶OÒ
,^AGN4FGL J0836.2+2141¿âåà1X'"@@'óUÎÀ:+?› 'À<b¶FxŠU@ìõ[â(ÿ@ö+ —ºœ?¹|ZÞr習"¼\‰/?Ôg˜*-Ðô@	õ½©Ä4"?¿É읢'½¿æ©ÛÑLŽN¿ébÇ«$ÜX¿å<÷‡¿ïtRQÜl¿íoÙ¬¯ AGNbcu3FGL J0836.3+2143MG2 J083615+2138?ïü¦Ã	Ú?1^:쏳°?:É鈙Ñ?1^:쏳°?ïöC%'7?RM˜šn•?Syµ®72_?RM˜šn•?ïìûÉds?P ^7Jqw?c6ôÌ?P ^7Jqw?ïöœ	iò?A…	Òÿ<?RÇí¦Ì\?A…	Òÿ<?ïûž¢J Á?=]9Á`ãá?A…w淅S?=]9Á`ãá?ïÓÊ(æ?vyÂ"t«?v÷LZ%*?vyÂ"t«?ïð$ݧ\ó?bon]bÕ
?_¶Dêÿ‰?bon]bÕ
?ïÕùg;t?f¼RË»À	?uLOaž?f¼RË»À	AGN4FGL J0836.5-2026?ËyÖ꡸¼@(9	(­ûÀ9ÞØ-SbÀ<&æ"Gp@rxJ"xÈ@¢|—*T?Ã([!?Ò7ö{ò¿¦@)È»ÆL@	ÒÀº컿ÝÑK·Žw¿ãŒk'fL¿ìæMÂ*²[¿ïÞï@4£¿ð?ïÿþBe«+AGNfsrq3FGL J0836.5-2020PKS 0834-20?ïïOã¥?uǺ?`ü°DÌÒÈ?uǺ?ïÖÏ.žEr?|ÂPà«Æ?t˜hº|.Ï?|ÂPà«Æ?îhŒ‰™Nú?žµ¯ÀE¬'?©w7j¶"a?žµ¯ÀE¬'?ïéŽ{DÉ?UúœLR=?fq"£"c?UúœLR=?ïêú>—aÓ?ld]R6½?eÁ<£,ì?ld]R6½?íƒÇÖBí?¾t_?³çñÀ?¾t_?í£jÛɝ?¢Ð[³Á?²ç̧×ؖ?¢Ð[³Á?îÂî?õIª?šÓ&¾l­?£Ñc3`?šÓ&¾l­AGN4FGL J0836.9+5833?à_Ú8α@BDaAcwŸÀ:ÆWꢠ©À<¦­@?‹0@¡¸Ðìl$@º:Þù;?¸a.n'z³íPÑ?ñ–¿Ê…Ë?ýq
×tp•¿ÜÏ|¿ïÒ¿áN
>¬ãù¿çh?ŸR@?¿âj4¼ .ß¿ã"2þ¿Ø­JÜKAGNbllNVSS J083705+583151?ïüì>Ïk?1—|\þ2…?? ™^5G?1—|\þ2…?ï즤o
¥?`€L-?cY[Âoºò?`€L-?ïéx4w´u?d ñð"]g?f‡ËrN?d ñð"]g?ïÕ;Ä?Vr [­Š?ubu_
y?Vr [­Š?ïñ±×(?SV`Q~î¸?\Ĝ–gúª?SV`Q~î¸?çD¥?€‰x`,?‹\F;žrº?€‰x`,?ïÜ'
ë?w<ª™ç'?qñ6ÀY?w<ª™ç'?î[Ǚ‡%#?"Ìb§f¢?ªC†eÕßÕ?"Ìb§f¢AGN4FGL J0837.3+1458¿ï"Y¥¢@>ȼœÓáÀ;)(Fp&ÚÀ<§p¶K@ ö
³\Z?ú'¢ê{3}?ÖÒ"4ÕË?Áéoo¦V?ñ¢.x¹OB?ý1D‹u>›¿ï±E½yr³?ï;ˆÂ0ç~¿éT•]õ©?5n&NHbo¿ÞëF'¿àª|uœdOAGNbllRGB J0837+149?ïþ¦º¥"
?€Bà?%"Y(hÍ?€Bà?ïíJ»\"]?pì­y?bµD†žëj?pì­y?ïæ_r¬Dí?iœ¿Âku?i q÷¢ç?iœ¿Âku?ïè…ñ­=!?Oµ,þ·È?gzc@ÿ;?Oµ,þ·È?ï÷p`D?V¨:/GŠ?Qç ¨ó?V¨:/GŠ?ï¯éGŠ`Ê?–—œu^T^?"®$öñm?–—œu^T^?ïÇ},Ì?'"R¤®pÏ?|Ajø9ú?'"R¤®pÏ?ïŒngõ?|ò^ÉèU?ŒúdXÆÊè?|ò^ÉèUAGN4FGL J0839.4+1803?îõZ»ê@?¶·ª%ÙÀ:`þU/ÝÀ<€VAU5@ùZ<a…@Ž±=û
R?¶Ðó-‰¦¿œ܃yË?å±
õ´M@»<.Y"¬¿ËßÀ‹t¿ÞZ~¦¤¿ä	`0Â?«¿åJŸb0w¿á•`Nõ1¿ÌBEÈa-AGNbll3FGL J0839.6+1803TXS 0836+182?ïþT­'†?•F~io<?*µ"Œ•?•F~io<?ïöÑbU,$?R?¢)ý~Â?R];٘·Å?R?¢)ý~Â?ïö*˜ý3ê?\e]Òl­?SªÍªâ|?\e]Òl­?ïû®üF%î?&k´Q¶ƒ?AD"Ø/2?&k´Q¶ƒ?ïü߅â?6úLTþ¥??aèfBb?6úLTþ¥?ïӞBÿ6µ?u¸)w&¹?v0Þax)­?u¸)w&¹?ïõÓtd^'?býcì¯-d?TY¸Ñ\Ç?býcì¯-d?ï©(á?NÃt¤k†H?a[Q0¶^?NÃt¤k†HAGN4FGL J0839.7+3540?ÄKÛÃ>f@BA,üœÀ:RÆvqvÀ<ozLÍ8-@ãÿ:³/B?þ¬€&+
?ºÛâ~å¹-?¶$[T ?ü§‡H^=£@çV:õ?ïþ7+æ8¿â¨Oªb>¹¿ÙÀ[¥B¿ÝP»>Z¿álšÈmÂ{¿â	P
ÚN–AGNbll3FGL J0839.6+3538NVSS J083943+354001?ïü1'j?1ûߛ?>syKH™?1ûߛ?ïïÙÍnæÆ?\ÒiÝ$ñï?`&2ž×©Ç?\ÒiÝ$ñï?ïî‹1QÝ?aEÓvò"?at÷ñ
;:?aEÓvò"?ï¹BØö.?aå˪š"2?¿oBã<k?aå˪š"2?ïõ?ìò?P9ÝÞ?Uú!…?P9ÝÞ?ï¿ÎS¬ò´?R\°Ú?€kÓð?R\°Ú?ïÙ¤Œïç?|æ煫À)?s-¹åªl?|æ煫À)?ï/…(É?'þÏÙ
¤6?œßº{®à?'þÏÙ
¤6AGN4FGL J0839.8+0105?ÙphJ
·›@8uà'Œ6ÛÀ9™'ÿùJÀ<Êþì@æAzɟÇ@î][$éÄ?µŽOŸ¶¥T?ȟ©érõÁ@ÂÇut÷#@~‹ž":¿ÓÐÂÛ\\¢¿à"0±x³p¿äSø:8àò¿æýNª‡þg¿ïþôx
¿ášXÜ:(AGNfsrq3FGL J0839.5+0102PKS 0837+012?ïƘú¤?tµ¨_"pÐ?|³ƒÊ_V?tµ¨_"pÐ?ïïëÏÁ‡?dŠ®'U¾?`0Ó£Pá?dŠ®'U¾?îç´Ò…Œ?•.-#Ÿxs?¡"²ÕöYH?•.-#Ÿxs?ïò"lf…›?C4ێ?Rî?[»'ì	?C4ێ?Rî?ïsLÛÐ˵?Œ4'÷=O?'–d‰V%]?Œ4'÷=O?ïÁ@Éb£Ó?'ò½Dj"i?_›MN>‰?'ò½Dj"i?ëYń6¹ƒ?«ú"Å:öæ?˜éï%ó?«ú"Å:öæ?︑g­˜?lžÈë]?Û¦
Á|?lžÈë]AGN4FGL J0840.8+1317?ç¾:"¥¡@>10ߛÜjÀ:"ÒÊ<ϔÀ<s¿T>E¶@¼è7"î@ᶃµ+Æ?ǜvXKñp?е£»[‹A@9E'Á@ÚEÚ)ו?Å?ïÚê¿áGïþU0¿èŒoz^Ù¿ä0|ŸÏ¿ð¿ïù^Æ^ô'AGNssrq3FGL J0840.8+13153C 207?ïîW»A£Ó?c¤Áׂˆ³?a¨D·|ôì?c¤Áׂˆ³?ïõ|ÀFÞ?V^"v¦bÈ?U€j¦‰?V^"v¦bÈ?ïž>3†.?'Qœ‰æ?ˆypyý¬p?'Qœ‰æ?ïø.ýïY•?3fc13?OD å?3fc13?ïöÁõ;?Vç•>ô8?R|}RT£?Vç•>ô8?ïѯÔ)Ɏ?y]$QMºp?w(è,¾?y]$QMºp?ï-{—Éz?'þŒÅ‡?šPŸÓæÂ?'þŒÅ‡?ï݈Ó	
+?]FÀ˜[âò?q;–%–C?]FÀ˜[âòAGN4FGL J0841.3-3554?çˆè>ö¾k@
î¦]¨À9ÃOu‰À;š$ˑc@ X¢õãÇe?øáS½vd?´kë
¥u?Ê:
Âá@d¼~ ïÏ@áé{Vw¿îHPÑ©«?ș5[+ŸÁ¿Ì}†éh¹Ó¿ÆÀUÛ~ÁQ¿Þâ›ìK¿çÏ,ù]OAGNbll3FGL J0841.3-3554NVSS J084121-355506?ëöˆ®Àa?Ã)‹GNý?À%ßýDþ|?Ã)‹GNý?ï>˜Ëht? `Έ_¼?˜?,ã#U? `Έ_¼?ì¥äQ^þy?§°iz##õ?ºÐÝu5?§°iz##õ?ï«Û'Oò~?pŽ‰7"3b?…	6,`?pŽ‰7"3b?ì=áêb¬??¸ä²¬"Á?¾ð¬êž?¸ä²¬"Á?ê¦U¡"‡-?ÈS¬tœ¢?Åf©y­ãJ?ÈS¬tœ¢?ìeºÏŸ:?¬&⸉ƒ?¼Ò)ƒ/D?¬&⸉ƒ?îi[…¯?##aŊ?¯ÙlÛZ
?##aŊAGN4FGL J0841.3+7053?â??dm	@A6T´:çÀ7ÃÜ«g!wÀ;ÁˆÛt´@±'!PÔ@2R¯')?"r×
•ž?͛¿«Q'@,2'1ìV@ Aa*½Bì¿Ô'Õ…-%þ¿å¦BWéK¿ëƇÙ}µ8¿íTÞ긿íäÓôß:Ž¿ïï ×{|xAGNFSRQ3FGL J0841.4+70534C +71.07?뙖òuRè?Èö±Z=R?Á™¤6*´_?Èö±Z=R?èþ³#ÙN?Ï-"ê§9?π3pšÈ?Ï-"ê§9?ç	å°Yµº?²øð—,Vö?Ñì4ŸL"Œ?²øð—,Vö?î·òëÍ÷x?­çÝ 3ۇ?¤€ÑAhº…?­çÝ 3ۇ?éAšÂAj?ÂøÆvù?Êù—ÌöúY?ÂøÆvù?ÒyØF†)Ù?ÑèÑážw?æÃܼë?ÑèÑážw?ê—Ǐ?´'µr긃?ǧ¥ ãåÃ?´'µr긃?ÙßDëä·r?ÈQ(DJe?ã]Š
¤G?ÈQ(DJeMIXED4FGL J0842.3-6053?í1_ÎÇ£ÃÀ&µÅäêÑÀ9P—2·qÀ<§z¡‡@*#ô&@ºÚâ9Eœ?±j=¶nçi?¸HçÐ^QÅ@1düÙÚÒ@U"–Ó?ïm­íät‰¿à/Z`ž¦I¿åt"狕¿â"ӟNå@¿åbUË
¯ì¿ïÿÑÜ×AGNbcu3FGL J0842.0-6055PMN J0842-6053?ïýé`	Ä?#¹Óbðü?0µXI7©?#¹Óbðü?ïó|vÕI?c^!ò6Ê]?YØÿ5?c^!ò6Ê]?ïñý¢­"?co5Zff.?]Ð'i‡I?co5Zff.?ï÷ÄÀ—gï?8öHÖ}Ôö?Pv~š6bî?8öHÖ}Ôö?ïý¬ú°›û?*Å­x‹Ü?2˜*|9¢Ð?*Å­x‹Ü?ïÅlǺ¥i?–é_ýEÚ?}Iœ6›Y?–é_ýEÚ?ïÛÉÆÌÇ]?xpk«%Yj?r¦ªÕP?xpk«%Yj?ïçÅ«½ªè?V˜ì;x4C?h:TXR—Ÿ?V˜ì;x4CAGN4FGL J0842.5+0251¿éóú3ô_t@9é™þCg^À;$r[UÀ<©F<û3@ @Öí7%†?þJÅ 0!?Ó͝aûÁ?¹%OšÇìé?á8À ý@VJyö¼
?ï')}§ËŒ¿ïH_	B?Þs[Ao6¿ßf'd@ò9¿ââÒÞßM¿Òä\Xp"AGNbll1FGL J0842.2+0251NVSS J084225+025251?ïÿNózƒ?¸
»£?#Þ7¼?¸
»£?ïôÿ)Z?Wül%7i?Vä)â[è?Wül%7i?ïø•x!Ð?[pö%g0?Oªwû}"?[pö%g0?ïô:ù¿ãÊ??S>²+õä?WŠ>?ìU??S>²+õä?ïÿ{vK"\?³»€·?'9pS»9?³»€·?ïÔúÝù'J?|§rÚAò??u''E^å?|§rÚAò??ïûTyZ4?Yè©`,Ù±?B­Â<¬ér?Yè©`,Ù±?ïæ¢è¼†G?X©4Ünœ?i]þÁˆî?X©4ÜnœAGN4FGL J0842.7+6656¿ì>úz–/h@AÎa(9.À;]u&ÊÀ<›ÚGÓ
@!®â‹ÐÙ!?ÿ`›KJ.?¼_ÿ™þ™N¿¯ž
œ µ?ðçáuÑ@\.Ìò¡¿â%NÂR ¿è8BÒ§®¿Å›
bE'¿æ½™Þ¸Ý'¿Ð'xB±ÖQ?ŒâèÂAGNbllTXS 0838+671?ïþtS}ÅB?Y¡^¢;?(ºÉ¯~å¼?Y¡^¢;?ïö$³Nݚ?Sß+µÂšq?S¶™9	|z?Sß+µÂšq?ïô ,Š~?d;Yè?W¿¦Í¢sR?d;Yè?ïùìù'@?4N^í–?HO¼«jp?4N^í–?ïý‰:¦Äû?/90!wîu?3¶,?­£¿?/90!wîu?ïÏ'¢}»9?€!K'žü?xl.¥¥ƒ—?€!K'žü?ïõDû‡ H?hnR¡–è?Uv€@ß?hnR¡–è?ï؈Üÿ[?i2ÕXÏ1|?s»ûü2¾‹?i2ÕXÏ1|AGN4FGL J0843.0-0853¿ã[€Ñ™@3ó)¡¹ù‹À:æž&Ç&À<ƒZ­ËÆ@0]^*Ü@^/æw˜¾?Ò'Y
]Q?ßëSàý±F@p¬bÉù´@	Jod綿Î<x{í?ßÅí οæµùìÀˆ¿ëÇ(}͋9¿£ CX´¿ïýè˜Û-¹AGNbcuPMN J0843-0848?ïüm¹ÁØ'?N©
Ú¥ÿ·?<'/î¬}?N©
Ú¥ÿ·?ïð¯ÁïG?]ô®'ò§?^ }¶©'¾?]ô®'ò§?ïsI-›n±?"å씤x?'–ÚI"è?"å씤x?ï÷íºƒ-??˜§F½Üb?P$‹|á‰ó??˜§F½Üb?ïùW"B¼µ?R_Gs ï?J¡ïqKÖM?R_Gs ï?ï°ªWàoJ?ˆfëTHíà?ƒÕj3Œ?ˆfëTHíà?î"LḟÍ?wç¹Î?¦Ë1èÁ†.?wç¹Î?ï»C6ha?wOGbØxæ?/<l6›Þ?wOGbØxæAGN4FGL J0844.2+5312¿½[ÚeØ@C÷…À9v}¾qÀ7À<QU>S"@×Àvþ?ÿðU2a|?ªß™ƒX?£¬Ð6f?ö²³"&k@NFæ™Q ?ï®Ê榓¿ßM™æÆs¿ãN4 C€¿Ö ËQ¢Š¿ä¹ø´²#Ô¿é6ÈééAGNbll3FGL J0843.9+5311NVSS J084411+531250?ïþÊúý?.ä• ¯?&óPª÷iË?.ä• ¯?ïößÚ4ƒ.?Püⵡ?R@LkBâ?Püⵡ?ï÷©f^P?X'»™"£W?P­ø½Ð0?X'»™"£W?ï÷ŠŒF°û??"À/D>?Pêç±ÖÚs??"À/D>?ïþtÆa´â?"t|°ù(?(³™HmK?"t|°ù(?ï׿¼îÞE?tš"Õ'?t !¢­å?tš"Õ'?ï÷^†H.?f²õÏÝ?QBóöT?f²õÏÝ?ïóW,%'¤?J'õ´8)?YQ§Þ;?J'õ´8)AGN4FGL J0844.9-5458¿á+€({ÁÀÿ«–òmÀ8Û}½›¢À;›ñþµ}%@|"©¶Æ@7G"ê?©b}=µÌ?¸?ëÓME@§,å;Xœ@¼ÓüìÐ"?èJB1}ѿڅ]à0¿áT¬?8¥
¿Þ_œ}y¨c¿äñÿ¦™¿é̪ÍÛÁAGNbll3FGL J0845.1-5458PMN J0845-5458?ïùVÆF‡?F²úiÄ9?KÂ¥³ôù%?F²úiÄ9?ï£çÌ`?‡,k‰_'?‡áGë?‡,k‰_'?ïË7z¯br?€Ý{¥I?zdB'QFß?€Ý{¥I?ï(!¤P¾?xÝZ@?šÿÛÍ-¶@?xÝZ@?ïغÈ#«è?u=gðü@Q?s¢›Ò­,6?u=gðü@Q?íÃæ:BWO?¶©ÖGÐÿ?±àÎ.É,‰?¶©ÖGÐÿ?ï	&єÌo?˜{²­#Ö?žÛ%ÔEª?˜{²­#Ö?ëNÛñ¿Ë?£"ÛÉא?ÂĐ9èÔ?£"ÛÉאAGN4FGL J0845.4+0442¿æ>{ÄO-@;lÁ"tŸÀ;OsۙïÀ<§7T*@NI.B^?ÿj`':O‡?Ϫ÷¥h"Ï?ÌûÊ;M?üÿ¦sœ¯Ï@¿P¸TE¿ïÿVø4Y¤?ïõ–àVÂZ¿áúØC""¿ßIMì¿æ¨ëÎE¿ïýøScTcAGNbcuMG1 J084516+0439?ïüÀ<Gž?0>y
v‡6?9ÿÝCbÝ?0>y
v‡6?ïïcgÙX ?`ZH!·Ó?`œ—îNGÑ?`ZH!·Ó?ïåÀú0h?UÍ%Ñ5";?j?ŸŠH?UÍ%Ñ5";?ï⌏oõ?P'õ\ò?mspjï2¸?P'õ\ò?ïûœ,Š¼K?>ÐÕÀð?AM¤!1"?>ÐÕÀð?ï ¿ú<®?€`H‰Ãx?~ïŸþ5&?€`H‰Ãx?ïÌã¢@ ?yÐ'nÈOi?yŽ.úú¦?yÐ'nÈOi?ïs敆ö?§9øò?'ƒ-O!.?§9øòAGN4FGL J0845.7-5556¿ïœqº¤ÎxÀ !¼jfÀ:‡;©À<#ú±¦@N§¯ÜÑþ@OIc÷ ]?·hã²°¿†–]¶$ÐÖ?Ï$ô×è?èE`üçi(?ïö€[¯ÿ¿à[7¹ª±¿æ÷a€£~u¿ãtUªV€¿ã}éµí¸¿ÕÁ›ì/>AGNfsrqPMN J0845-5555?ïõó†ÂHÝ?QÔèÊæ5?TòA´Öæ?QÔèÊæ5?ïRûÐùàµ?¦0ú yðw?• …ßk?¦0ú yðw?ï°-bld`?'|荺i¦?ƒô§kn*?'|荺i¦?îƾá°<?‰É£ûÜՐ?£ž¤	<?‰É£ûÜՐ?ïÇD|»Š?}óâ?Aµµ?|]ôáîŽë?}óâ?Aµµ?ì]ðd,?Â2Ùº¶[?½$ßn¡?Â2Ùº¶[?ïcÊíFt?"ØŸP?"†¢W>'q?"ØŸP?ç؂ÄÚ©É?´	yªª§Î?ÐNúvJ¬n?´	yªª§ÎAGN4FGL J0846.5-2609?'ê•K€Ö@%(:û~'À:ž>Ü´¡]À<)›ûs©@"	ªÎ @jÀÒÄ?ыì\ßÿÚ?Þ&S0/@K}\L11@Àíñ_©?¡©³m¿Ù™·@ôfð¿âm5Þ^s¿ë?nu(¡	¿ïÿöût€?ì.¾ù¥sAGNbcuTXS 0844-259?îí	"íý
?¸Pµ0ÒE?¡/f®Œz4?¸Pµ0ÒE?퉬ælIï?³=OÁ´?ã?³²˜Í¤?³=OÁ´?ã?íqÒÏ+‡ÿ?žŠÀŒh?´qi†5̆?žŠÀŒh?íšq£0q?•(Ê͹ÉÊ?³/¤pÀºù?•(Ê͹ÉÊ?êùŒÔ—Ïó?ÀÏmEӞÎ?ÄÌ­ À2?ÀÏmEӞÎ?Öέ¿Ál?҆ÅÊø?䘩 9J?҆ÅÊø?å0žfe˜>?¹þÿSØ?՞Ã34τ?¹þÿSØ?؅bgJ´Q?º"‡ò'OO?ã½NÌZ¥Ø?º"‡ò'OOMIXED4FGL J0846.9+4608¿ÒÊ®aI=ƒ@Ce]€ä–îÀ:Ò}qDçÀ<–¦¾EJ@	8NÐóx@Ü{£åLö?ЩoÐrt?Á–ÌR֒?ë¹óêH@qð]J´¿Ö,DA"Š¿â݀y7$¿èÌOÏK,N¿éàkB"#¿ïÿÛ¢¨‹û?ÈXp™ñaAGNfsrqWISE J084734.29+460928.0?ïþjwϲ?($‹þåôr?)X›ª>·?($‹þåôr?ïóòÑ`õ?[lè_Ÿ'Æ?X^·5ç?[lè_Ÿ'Æ?ïè0·ì/?[M€cU ?gÏér®øî?[M€cU ?ïñóm©x?D·1…¦'v?\$>a(?D·1…¦'v?ïýªvqÝy?3M¢P<É?2¬M«Š ?3M¢P<É?ïËÂCºr‹?yfm*ys?zÞ6Š…?yfm*ys?ïÅÎÛ1?'7Úê4M?}{˜ïÓ÷‰?'7Úê4M?ï"5n÷¯y?y¥}׬Ã?‹2¤7ÅM®?y¥}׬ÃAGN4FGL J0847.0-2336¿íSu̜ @(hïܜM©À9×u;À;Þv˜Ñ @©lut ?ÿ
ÈÅ×F?§øä?'›Ú¶š?ì[?pé!@ƒÃŽ?ïÔv_î¿ÓŠ¬–Ì_À¿áGOµIùH¿Ý¹IbI¡4¿ÙËÿ€>T¿âØÄL0ZAGNbcu3FGL J0846.9-2336PMN J0847-2337?ïüÅPè·?/­:[¡Ù«??‰ÔïIé?/­:[¡Ù«?ïét,˜î?mê‹jó?f‹ÔB‰Œ?mê‹jó?ïïd-já?guøă?`›ÒjƒÉÿ?guøă?ïã@ùç¯t?Yhñ5­Ñ?l¿ œ]?Yhñ5­Ñ?ïó;ã?Ö?PKMl€—ü?Y‰ÃÜ
ôÐ?PKMl€—ü?ïˆbìx'ž?—¡c3ùN-?çDކ|"?—¡c3ùN-?ïÕbójEn?}¡-p­M?uN†`ÚÈÒ?}¡-p­M?￞>ÖÓ?p½íê\]W?€pI3Q?p½íê\]WAGN4FGL J0847.2+1134¿Ð%Pʦ_ƒ@>æãK"SÀ9꣩½ÔÀ<#¥©rU@ þy{Añ?û4<G®ë?´Å"Z‰?£"ö>,­Õ?ò7g«
f@ÀÞöÅð¿ï½µ¢ä›ö?ïþi'jÑ/¿×JC˜e¿Ü¯ÎD¬¿ÝXÏå[?ŸÐňhwkAGNbll3FGL J0847.1+1134RX J0847.1+1133?ïþ¾°ï‡?lV]š?$íÑÿt ?lV]š?ïõÏ'΄?WuÅY?UÔaýZ8"?WuÅY?ïõ"È7wø?Eòá†)?Töo†PÜ?Eòá†)?ïó™¾
DÛ?BžÀÆzýü?X̃ëvIø?BžÀÆzýü?ïýUC?.
ΰŠîœ?5W$ܨå?.
ΰŠîœ?ï΀­©4Ü?xüC'&Y?x¿©ú?xüC'&Y?ïí"ၘO?qX¿]L?bk=Ï	»?qX¿]L?ïÞÐT¨Ë?aç=å‰t?p—ÕæNB¡?aç=å‰tAGN4FGL J0847.9-0702?Ó\Áع%a@5ø`»+º™À:xºüÀ°À<dÂI¼´@úc"9:ß@°;#Â|è?¶ù¥rë¯ç? @½+ç\?çÏAò×s@ÁÔÜ:Óæ?Í>^!"¿×¦Gݏ<ɿ凾s˜©¿áè<à8Ï¿ä ©¡Nš¿âÎ÷IxAGNbll3FGL J0846.7-0651TXS 0845-068?ïûvº¶8¥?27erëa?B%Äà€?27erëa?ïñD¥ÃÀ×?]X™òI{ü?]v³ú²Ö?]X™òI{ü?ïðYqí7?ew-@"'}?_Mca?ew-@"'}?ïé+|Ü
?N⻚+?fÔ~?˚ç?N⻚+?ïó!7ˆ,Š?N@æ7Qaº?Y½çgÜt?N@æ7Qaº?ïÇu•¶é"? [䆰?|E5,ÊEÙ? [䆰?ïåÇÐlG?uôHϝO?jè8
wñ?uôHϝO?K¶'?rÛV7¥?‡­ɳj?rÛV7¥AGN4FGL J0848.0-0524?ïG>à1ü@6ÛíúCþ]À:À›f"À<cþë-
$@5?Ìt@3i3 @}?ƀB¸â4?¿v
xc"ù?ô¢ŸÒ˜¾¨@Ô
UÓò?ï-©¼&Œ\¿é¥Œ#Wô¿æOÿAi+é¿ï*Ú~çÆ¿ï¡3Œ†Ô¿åT/aíZâAGNfsrqPKS 0845-051?ïü­¢åó?8¨dIÊ»æ?:'é3XD¬?8¨dIÊ»æ?ïàùû@ý?}'ýåõÆ?oZ¿?}'ýåõÆ?ïÕBRg?v{%°&Ņ?u^þk"ôO?v{%°&Ņ?ï¾áóX/u?fOº'?€Gƒ4BöÌ?fOº'?ïôö¥@õF?`ÞҞËð?VµÞJ'î?`ÞҞËð?ï~}#l@Æ?™+ò-KÁ?0[P}I?™+ò-KÁ?ï·)É
`Í?'Ý6™Š?'5º@Í?'Ý6™Š?íõ§À"-?™#hÆu ?°RÂ! ?™#hÆu AGN4FGL J0848.7+0508¿æy
Éî²@<Zþ`Ï6À;U$H¸À<xæÞÆÊT@"øàå³x"?ù·Ab ß?ÙC«QÎ?Á"¼:-x^?ð:CȬ¬œ@ߢ8y™¿ã^V݇Z'?ïƒ}ÎaøC¿èåÛ&+ã´¿á:À›;/¿Ë¡£é©§Y?ÉqŸÕrã¢AGNbll1FGL J0848.6+0504SDSS J084839.66+050617.8?ïÿ;xÀÊÐ?ƒÄA+—?æúžù?ƒÄA+—?ïóΡc<?Xyv݃³'?Xb¼»@?Xyv݃³'?ïô‹kD_?P™ïÛ?Vé*9.0Õ?P™ïÛ?ïú*¼Ó@À?8Ó]X/Œ?GUšÌ‹?8Ó]X/Œ?ïÿór´?<åŽ¿Ñ?""I!?<åŽ¿Ñ?ïÐØèŽõ&?w¥¸xçN?w"‹ËPø?w¥¸xçN?ïïQ©ëÌA?j½Àx'Dm?`®UïöÒ?j½Àx'Dm?ïØà–Ùì?q¯^%ôâ
?s´›¯È?q¯^%ôâ
AGN4FGL J0848.7+7017?ìg—á*@A—Ô{í·(À:£`ó_ލÀ<½ùŸ"®ž@ 
ÜkÒ6?ýDãü";?ŞÜÏyOw?ÍvBýU«®@ÄÛÄ·T–?ÿȃßÈýà?•¬g@o˄¿æŒKgÝ^ë¿Ø'(üùe\¿×m›¤`Çì¿âƁY0ô¿ïÿxPsµÚAGNbll3FGL J0848.5+7018GB6 J0848+7017?î-²Q/Q?ÊLGÝ jÕ?­$Úêl¦å?ÊLGÝ jÕ?ïϖψe?sól/q™?x4˜u›¥E?sól/q™?ïÆ-é>¿Ñ?zzƒ|hZ®?|é]0{¬?zzƒ|hZ®?ïRæ=|?v÷Ö~7ý?œõ£1}8€?v÷Ö~7ý?ïœqЧͺ?¡ÜęPO?ˆã‹Ï-Y'?¡ÜęPO?ï$¶}ð?š;§(w'?›~é-ðB?š;§(w'?ï(tߌ(S?–Œ,g^?šñd¢_–?–Œ,g^?뜬t£Ò?Ÿýዮq?ÁN-p·´?ŸýዮqAGN4FGL J0848.9+0205?äMˆr9@:îU7«À;(&x9́À<'IÅEïÎ@sñÀ¢@"ę?ÔÀü§…ë?Ån"›þ£´?ó?ª¥Z—ü?íqlŠ†·?ïøgºú<r?Պt";¿¿åüfîK¢–¿àÇ&/>±ì¿ïè5sS¿çåÇ°å;AGNbllPMN J0849+0206?ïߺ}iã?wÍ1ÊÈþœ?p"Á5ÀÝP?wÍ1ÊÈþœ?ì}ïmûIý?º6È 1^?¼"%°?º6È 1^?ïZ&6´?"owÃAD?žt»?÷z?"owÃAD?ë×ê¬$â?ž£ö<å?À W¹Olz?ž£ö<å?ï¹ÀÌäJ?ƒìgðrU?»OÝE
y?ƒìgðrU?݅Òj¤S?мåËïº?á=Ê­ô×?мåËïº?î€ozûã€?œwƪÁ‡?§ùS±d?œwƪÁ‡?ÚÕ Á:ã?µxä'fN¦?â•/ŸâŽ?µxä'fN¦MIXED4FGL J0849.1+6607¿Òэ{ÔÛ@B7•=êFZÀ9î.C	jÀ<}Œ†‹ŸÜ@qd<ëmÍ?þӀ*\ÊÜ?³7çßï?£Ê© ¼'\?ñpÄÃéÏ<@	B6n&#U?ïýå^0´¿ß¿ziR©ñ¿â"~§¥Ì¿×™ÒduÄ¿á‡.'ŸW¿Ý×åÐDAGNbll3FGL J0849.1+6607GB6 J0848+6605?ïþdzTÎ?Þ=e?#"ÍȒ¸¬?Þ=e?ïö¥'þD?T]¤µ|Z6?R´ùâ{«?T]¤µ|Z6?ïõXÂ8õ?crÂΜ߸?UN{e("?crÂΜ߸?ïñG5Ò'ˆ?D–ÚN&É?]q"ɤnø?D–ÚN&É?ïþT­'†? £îtÇV?*µ&=°}t? £îtÇV?ïÔH­ª?}‰IØJ¶0?uÛ©'ŽáÆ?}‰IØJ¶0?ïôõ U p?g£JÓ¦ñG?V¿Ɵk?g£JÓ¦ñG?ïàD‹ 1¹?[ãngý@c?o»t7òÏ?[ãngý@cAGN4FGL J0849.4-2911?ÓX(+ö²@"nf¼˜¢À:¼i¨:FÀ<=MéDÓ@Ï`¾1@heD'w?»@DÔn?³ëÉ(]±?ú
üÈ=@|U\'ô?ïþ!8^ì¿åt ñ|¯~¿ß¢ûB+¿ÞžÔw
þ¿àG†Â&€¿ëˆô›GïƒAGNbcu3FGL J0849.5-2912NVSS J084922-291149?ïþJõ,ùn?¸õ"!M[?+P¯fHÖ?¸õ"!M[?ïåÎ,¥7?sY
¥‹?j1ÓÅa	
?sY
¥‹?ïóEœcÅÅ?i7ÙÀc"ˆ?YtÆã>'R?i7ÙÀc"ˆ?ïú:zFº?-Ÿ'§mù?Gƒ&$?-Ÿ'§mù?ïþ
Ä[0 ?'IS÷þÐo?/#ºA÷E˜?'IS÷þÐo?ï2‰à¾ò?¥ë'·Ç0?™¾Â0S¿?¥ë'·Ç0?ïò¹c
–l?hgÐÊa{Y?Z9yŸYq?hgÐÊa{Y?ïðçíM­?G'Á瑾Ò?^0%Ró?G'Á瑾ÒAGN4FGL J0849.5+0456¿ì5ùø0K@<pÊ>}QÀ9×KÞ$ãåÀ<#)è0Öb@‹v9@îš|îh?¸æg¨…ŧ?¼ªŠ,¿%Å@ዻŠ…*@ÜÁ]Wõ?î™dÀsøö¿ßÈy`¿'¿ß"C")m¿ÙDÜޒȿéA¢a¿7¹¿Ûlk"¸¼ AGNbll3FGL J0849.3+0458TXS 0846+051?ïñ·!Œ9+?XD¸ñ!?\'½J'hþ?XD¸ñ!?ïÚý³ZÇ?sû1$¶?r&dztW?sû1$¶?ïÊv<-"ó?~¼@2ÙÚ?zÄáð>e?~¼@2ÙÚ?ïPšÓ'ž4?t(‡žE?•ì¥…53"?t(‡žE?ïŒÜ½ŽI?‰š¿]Î?ŒÈЪ,,ç?‰š¿]Î?ï{ãœP>?œ'	ñÿ?ƒ'b+?œ'	ñÿ?î)†o#?¢š¾:kic?­g™‡¼µ?¢š¾:kic?ìÆ\•q?˜>æÕ•?¹ÏíTwÚ?˜>æÕ•AGN4FGL J0849.8-3541?ï¢Úú¦¾Š@ßãß8	\À9"8½¶¯TÀ;ºƒDÃ~o@X®ýÙà@eø5/?·;F}ù}?ĺ…aÿ#Œ@	ÂJ'k~Ô@Ž–±1ç?é¯,ÅÇ¿á–kðL¿àÈÔ_"8¿åþ†]§¥÷¿ë]Ñ6¾Øî¿Ì[ª
U‹AGNbcu3FGL J0849.9-3540PMN J0849-3541?ïêMõ'yü?c•Ê#ô°?e²
^g¼??c•Ê#ô°?ïß(ԁïP?}dôÌõ)v?pk•Øus´?}dôÌõ)v?ïC«õÖu1?É5'=m?—ŠE1Yâ?É5'=m?ïùç,Þ?1R"´ ]·?Hóõ9™?1R"´ ]·?ïÂZ¤LŒ1?x…ˆ±
*?~Ò­Í[O ?x…ˆ±
*?îÕ:B¥?­Lf@=í'?¢¯¾ëî·?­Lf@=í'?ì˵™+ ?ª"Ûyæ]?¹¢S7Ʀÿ?ª"Ûyæ]?ïèÑhpŠ_?Rj"Ky?g.—z×øÕ?Rj"KyAGN4FGL J0850.0+4855?åØ^Z ¬Ö@C¢õ#-+²À8¬ß½jY:À;åùɅ°@ðI°ù½@Ê]†ÃÔ?¢E!Œ¡?«}~o`z@¤ûÍkX@?X@]é?³­L¿KYñ¿ß^y½±%ý¿ãI_à:gÛ¿ãú*~å8¿å±öQo^¿å8!WnAGNbll3FGL J0850.0+4855GB6 J0850+4855?ïó踙A¹?‰œwôO€?X.ŽxF?W?‰œwôO€?ïöMˆ/J,?RµƸp%?Sdð ¸?RµƸp%?ïï ½¶jœ?jrq'Z?`_BîûË?jrq'Z?ïþÝÅ\Yâ?'Vvfj?"#«.yS¹?'Vvfj?ïþƒ˜ü:Ï?"ÂçaÁé?'Æm`ÁÞ?"ÂçaÁé?ïÒù'¯Ø†?~|ÊkÂ?vƒl7áð­?~|ÊkÂ?ïãÆá¦M²?sݺl`C?l90vþ*?sݺl`C?ïþDÿcwõ?"7&g/Õ?+°Ð_‹?"7&g/ÕAGN4FGL J0850.0+5108¿Üþ‡µ	¯@C'û îÙÀ8¼$>úèÀ;üyx'â@æzšÆë@IzŘûå?¢ïÁÄ[D?µC;&x@¸ÁƒÃn@§,_›–¿Üo1CD¿Ý<+)yv¿ä0usI¤¿äûR@ê€è¿æ†é"¬ðŽ¿æðc?jyAGNNLSY13FGL J0849.9+5108SBS 0846+513?ïýG4¼í?,ê´æ½hö?5ÇTÂ-\¬?,ê´æ½hö?ïöêR?Tn÷«±íÎ?Sùyøͅ?Tn÷«±íÎ?ïè
Ë'õ?i×UÉ)Žù?gõ4»³×?i×UÉ)Žù?ïÿÌý°U¯>ðLÿ4>ùø+¯Š>ðLÿ4?ïþŽ¯õjj?ž¬óŒ
€?'þkgvH?ž¬óŒ
€?ïÓ-›]'×?{¬wRaƒ?vi2`\܄?{¬wRaƒ?ïèlY´@(?um®ÊOdW?g"¦'¹—â?um®ÊOdW?ïÿº*2Ùq>ûÄý®•¡â?up›‹US>ûÄý®•¡âAGN4FGL J0850.1-1212?ïË_r^õ·@3‡U¼Ê÷
À8w1ÅÀ;Ê+"Ù@y@¹åCç
'@<†™Õ?£3ìk£'?¶tJՑA†@pO'RÑ@ßSŽê"¿ÓW‰ÿ¯~¿àæ¯â[Te¿ã‰»€Hj¿åãZb¢®¿éêk
•ù¿äna|òšAGNfsrq3FGL J0850.2-1214PMN J0850-1213?ïùõ†C?_?A`ûŸ?H)æjsr?A`ûŸ?ïïb©Ëôh?g")ŒG¡×?`VOˆwŠ?g")ŒG¡×?ïÜË;äC?oŒüã`¶?qûšv«†k?oŒüã`¶?ïÿn
RFý?d†k'?>³1vä?d†k'?ïú\Íè×?B]%;O?FÁxH¤©?B]%;O?ï²h±ÒÝ?‰ÚlXÔé?ƒeø ™ÌÈ?‰ÚlXÔé?鷺öû8_?Œ<öŸfߞ?†ÑB3sx\?Œ<öŸfߞ?ïþÁFåJP?	/âia?#땈ê"?	/âiaAGN4FGL J0850.5+3455?ïúk²fÖ4@CHå£]gºÀ:RLƂ/ñÀ<‰I÷šÖ°@ê3ß*b@M~ˆœT?¶ç\20¿"_! í)?Þìì\µ½@[œúø\?ïý!ÿ.Hé¿âP_("ƒˆ¿àö¾È'L¿Þ¨,"mb"¿à"Ã`èM1¿Ò|Óz»ÝçAGNbll3FGL J0850.2+3500RX J0850.5+3455?ïü±8iv?+'Zð²Þ?:v;60z?+'Zð²Þ?ïõ"Fˆy?UKZxÀq?TÙshËM?UKZxÀq?ïø;v+^?=›Éµ¼kH?O(cr?=›Éµ¼kH?ïôÈ~ßY?<½óÁi<?VoD
ƒ?<½óÁi<?ïû³WäK!?6CÇ2·•â?A2 D~±'?6CÇ2·•â?ïÐ0'w™ó?zdN…µfH?w綿c'?zdN…µfH?ïòg¼…_ƒ?j¡ŒÊW?[0‡1º´?j¡ŒÊW?ïà£gè`k?X" #€ÿ?o\—ïÄO?X" #€ÿAGN4FGL J0851.5+5528?Í#wb{äí@CsàâiÀ9ÜE ›€úÀ<Žv3cÛ@|"œT‰ð@]ŒzÍ%¸?²4<ó{b?©ýñõž?õŒSâÖ$@
ð%a¹X|¿±ùiã-¿â¢TˆîP«¿âX._ŽÛпâö²ydp¿ãâÔ}›6¿ç÷Àá‡AGNbll3FGL J0851.8+5531GB6 J0851+5528?ïþ!̓0?!žÓÞúT­?-ã+Ò€Ò?!žÓÞúT­?ïös9>ï?Q­ÆÚ¸z?SÅÉûB ?Q­ÆÚ¸z?ïö³ì^Á	?`óæcA-ö?R˜'J¼ý¥?`óæcA-ö?ïõjL'˜?@îžô²À?UÇ+iºª?@îžô²À?ïü¿ÛŤ?4ÅI¸?:#ݹ˜r?4ÅI¸?ïÙà}r‹R?qúq~P¨?sÁg¶—?qúq~P¨?ïõñm"Ø?e‹{£)ZU?UÖ¦' D?e‹{£)ZU?ïãQƒ«E¾?W~?c~½¾?l®|Z9¡}?W~?c~½¾AGN4FGL J0851.9-5229?åXÚÕ¬¢éÀ˜e"™‡üÀ9·üjIJÀ;~ðW‹@Ë`V{@ä¬{*C?À"'$17°?ª9Ò?ìÊ/ßÏ @	?âTžgà¿©÷؂ý9Á¿ªK̇,¯‹¿êòÇhýÖ¿Ûçœr<¿äÎý>.¹Ò¿ïÿ¹ß	eYAGNbcuPMN J0851-5228?ïýK͚
?/}šð9Ä?7] a…‰k?/}šð9Ä?ïì仒#?rףּД?cD‰YËò?rףּД?šâïÏ?Šm±#òû?‹\YJ³¨E?Šm±#òû?ïø]Â()?3I{®ZÑO?Nˆ÷ïoÖ±?3I{®ZÑO?ïëÆq¶H?hЦ
nö?d9ŽFø2'?hЦ
nö?ï"~'ÅuH? 	ì)é?‹ _DSÚ? 	ì)é?îÆ9óõ8Y?Ÿt9žîSk?£œ`¼`÷o?Ÿt9žîSk?ïÓÁæ"Éü?e Ð­r"?vÌHmÚ?e Ð­r"AGN4FGL J0852.2+2834¿¿ëGC,òÊ@B×ÆÁ#À:]ÎpÀ<‹	%B¯¨@üܞ&H@'[··?ÆBèé­?ÂS7Q¥å?úåW¨]»@æèî–v$?ïÉ,«¿æì-_ߎ›¿å
ñáe¿äˆ—³æKú¿ð?ïê
_ÕR­AGNfsrqB2 0849+28?ï暣ڻ"?dÙ¥~y_—?ie[è˾T?dÙ¥~y_—?ïè!UKr*?hyXäL5?gÞªÛ	uP?hyXäL5?ï ÛPYoï?øQy#×?‡É+ßU0K?øQy#×?ï¼úp/N2?iªÆýÔÑY?€ÁcìOl?iªÆýÔÑY?ï'䉊Ù?›šÿ
¼»j?›~ïló?›šÿ
¼»j?ïaeÌJs?–gÙE<[?"ÓF}V±¬?–gÙE<[?îãÖ
é!Â?›=Y!»Xß?¡ÂŸ$˜Û?›=Y!»Xß?íéQZe§$?žb¿Ø^¾?°µu,dÓb?žb¿Ø^¾AGN4FGL J0852.5-5755?Ú5
Cñ' À!	3ã\[KÀ8j$咖pÀ;ÁŸr ¯@uƒ°Ï@J߈'4?¢àÏqì=?¹8Ñ,ØÑ@k"˜€"æ@r'M÷¯¤¿Ùg*±"r¿Ý÷"[nç¿ã·ž'6¦…¿ã¶°@O%'¿ç>Õ]•¿æ²\sž]NAGNbcu3FGL J0852.6-5756PMN J0852-5755?ïû聑Õ?8Ni½O¤?@]ù—õla?8Ni½O¤?ïíni%n¶?pë/гzV?b'–ûŠ,?pë/гzV?ïä»þ•¿?hõþó'–?kDŒá?hõþó'–?ïÿÃ*üFÒ>óLLÆpə>þj›pfêÓ>óLLÆpə?ïüÜ;NO?1ÃÝ^—?9ã7ßH?1ÃÝ^—?ï~8ñt]0?¢®ýiXÑV?8áνü?¢®ýiXÑV?ïÕfh·?'}ÎÊl?uL˖#|?'}ÎÊl?ïÿgÔ¥‰<?·E†êì?gøN&?·E†êìAGN4FGL J0853.1-3657?h2Ð	á¶Ú@°hÀ9/²Ä
ªÀ;ӆžë2@ ­"Ýõ¿?þüÕ©`à?±upÅ?¯Ql^YR?ü˜.•>Á@ĖóL}¿æ­§"n>ø¿ÛžÔA
aX¿à
fÀÿ91¿Ú-'	'`¿â g߿݋c`wAGNbcu3FGL J0853.0-3654NVSS J085310-365820?ïø|f`À?G›u½/&?Nem3D?G›u½/&?ïÊtOÞ¿?''SR ?zÅ×õ{Àá?''SR ?>·™<…?'ÕBf%Ԟ?€ØR è®?'ÕBf%Ԟ?謁´¦»@?o¢'ÍP³?…PÒÅ#$?o¢'ÍP³?ïݏœY??h:°Š¶Ï£?q81åÍD,?h:°Š¶Ï£?îr̳èü?±"\ñÅ#?¨Ó4̹¢;?±"\ñÅ#?ï~-S0Ñ?…!Øæã.?:U–~iå?…!Øæã.?îRI=q?˜áÝ|³´í?ªÞ‹màAï?˜áÝ|³´íAGN4FGL J0854.0+2753¿ìgÞÚÁW@Bóâ?$ØýÀ;þ—ó§,)À<öÀ
¢€@#kȂ»0ÿ¤¢F…‰A?ææPaAcx?ïþÿÝÑ@‹{ɤú@ûëLi»?ã&O?XZŠ¿ïÿßÿY'í?ïöü´>?Áâå¨eå7¿Ñ@Æcüÿš?Ô'»/ìVÖAGNbllSDSS J085410.16+275421.7?ïï¹Ë,'•?a&CFâÏ?`F4ç:Ü?a&CFâÏ?ïõR0¾'²?V‹çû_…ï?U[žuò+ž?V‹çû_…ï?ï8ç?W?'î#ÝËdÒ?˜ü£T‡?'î#ÝËdÒ?ïöÇätx?G1 /´œT?Rp7KIî?G1 /´œT?ïòšBG3?a©‹ö¨?ZË{¹Ü·?a©‹ö¨?ïÐ"	ó§`?v³/8?wîûêÀ?v³/8?ï'	l\Áï?Zã|'+?}¤ÛB?Zã|'+?ïü¥-Ìl?BÝx¾üá
??RՉº¡x?BÝx¾üá
AGN4FGL J0854.3+4408?çún_rðý@D5~g,À:ÎKUhè!À<œ™ì¥°(@ô-.?÷Æ ÆI%
?Ŭ§¾J~?Ò¹]XJÅ@s]Å­ôš@Æm°Ãi¿ïþÞAê05?ïçè絆_?Òç¦læ³(¿Äbl†»ñ]¿çFm!ÁpοÖ5I£bQAGNbll3FGL J0854.2+4408B3 0850+443?ï²"½·†?ˆð‹ûÑf?ƒ~›¡âx?ˆð‹ûÑf?ïÊàDè"?|ì"ë:4Õ?zÝ©ûþÊ?|ì"ë:4Õ?îs{Œµ§å?›'JIY£%?¨ÈG2Ì»?›'JIY£%?èÅYo?r¿Mó$è©?VՈÜS?r¿Mó$è©?ïD‡!$›s?™ÆՅ´ß?—oâKɉ?™ÆՅ´ß?ï¶ä"P?«äqâ¤?ß)*L­ù?«äqâ¤?ë\.)3*$?°7šœ?G[3Wp?°7šœ?îZ}µý?˜±@üµÍÌ?ª_(ʖ?˜±@üµÍÌAGN4FGL J0854.8+2006?ëqQct*@AéÈ!laRÀ7'm¾iÀ;Y'àðp@@Öòj–!@>ü½U`…?"ÏÞF"0q?ª;·²@ºKÛ ¥'@£ñ
ݜ¿Äõ;Uìq¿àÍS‰Ò|¿ãá~ ›¿ãD_÷6ƒ¿æ²¥­Û¿â~25r
AGNBLL3FGL J0854.8+2006OJ 287?ïû·‡|qÒ?>@èîÂMô?A!âƒÞ‹¥?>@èîÂMô?ïóÓ»˜5Û?_Ž.Ž)?<?XXˆÕ©¾?_Ž.Ž)?<?ïá»
ú?rœ`¢Çà"?nDòm±6?rœ`¢Çà"?ïþµÕ0ëÓ?Ò¿P;)?$¢¯	Ò V?Ò¿P;)?ïý…Ý'°'?+î–"1?3Ñ*þy×?+î–"1?ïΈ^]ÙO?}]@=€ì?x»ÐÁõŒ?}]@=€ì?ïí*ô?sx2/c?b€bÙ›É?sx2/c?ïý<ãyü4?/Á•‡—Ä?6âd…Ô?/Á•‡—ÄAGN4FGL J0855.4-0714¿êœeûÊ@7hëíúCþÀ:ÒdcVçmÀ<wÃیƒ1@ÑÑ¿¥ÇÐ@…ïbùÊ\?ÌhP ~Ж?Ø*´ÿ¦"Ó@	é{Y<²@!­ûü:N¿ÜÍ<žÁ̔¿Òþ=Áç¿ã¥Í"'± ¿ê9QZe§¿ïúÞ°ô?ïua Va¶AGNbcu3FGL J0855.2-0718PKS 0852-07?ïΑHf°?£—¿Zæ"?x·[Ü´I?£—¿Zæ"?ïÄxçŒ/"?‰¢NÏÿ?}ÌY"ž'?‰¢NÏÿ?ïĉåÐ?'7)ÊÅ?œGnƵ›(?'7)ÊÅ?ïÅ«ÆEI?f'ã	‹­:?}*t=ٛ8?f'ã	‹­:?­2.?Š=Óڏ"?‡™"©)`u?Š=Óڏ"?ío
ϼÁ<?¼GÕùé‡æ?´‡©ƒÑÄ?¼GÕùé‡æ?éAý‡ÄsÒ?µž01ñÌ?Êø	àî0¹?µž01ñÌ?íxvÛöر?¢Àæ Ä—Z?´<IÛFö?¢Àæ Ä—ZAGN4FGL J0855.9+7144¿çÁMm¤¦Ç@AŸÄ~I±ûÀ:=ʝG¤À<H³B¸u@ñonwØ@§ú D®†?Éæ\Ukl`?Ÿ‹™·Ý¸"?Àe$w®@	"¤èWAÛ¿©…Ðäßh¿âõ°¡š¿èÃÜ-'àB¿ã¡Mø±W&¿ïÿÈ!ÂGŽ?ï÷A)@AGNfsrq3FGL J0855.4+7142GB6 J0856+7146?ïüs–Õ*?3wn|·?<g	'¢)~?3wn|·?ïö¢S
¿?Sˆ
™0i0?R»ïNëÂ$?Sˆ
™0i0?ïêõ+»›?dê:Vã?eô
фµc?dê:Vã?ïúÁ0{6Ç?3¦üޚ¾m?Dû=ª$p?3¦üޚ¾m?ïþÕù#ö?1~¿^Œ?.ҝtãë?1~¿^Œ?ïÒñɨÍa?z'`á¿?v‡2x‡­?z'`á¿?ïì÷}á"j?mÖf ;Rö?c'X& ?mÖf ;Rö?ïãÓÉ7¹?`È~À,?lê,kVk?`È~À,AGN4FGL J0856.4-5309¿Ì38bXKÀ3éBNY)À:™ÝLvÑÀ;õP~"Ñ@ "è[ôs@fq%Ý	[?Å%'Abu쿆:¾üpÔ?Ånø_»Q@ÇÔ/‰?éíÊsV8ò¿êѓ ÔÇ¿ç³ß@ñ¿åJZ«¼1¿É24/²u3¿ä3ÝbFF5AGNbcuPMN J0856-5312?ïúczñ\?Fêmðx©?Fr¼cw%?Fêmðx©?ïí°,X?q!¸ÚÐ?bO€tó/­?q!¸ÚÐ?ï镯Cé?h Ze,Ò?fjPž°‡*?h Ze,Ò?ïûÔ¿+ñÃ?(º&|‹?@­5ՎŸ?(º&|‹?ï÷iôô?Djmë²ä?Qç-fa©(?Djmë²ä?ïx¥ç
sd?¥Ë_Ü«ßd?ëC 	aˆ?¥Ë_Ü«ßd?ï×ÈÃÜ?|»a"›*÷?tù›žà?|»a"›*÷?ïâ§yo?bXØÝÉï?mXç$¢XÓ?bXØÝÉïAGN4FGL J0856.6-1105?ïÏÚpç"@5y*0U2aÀ8‡¶Šk(À;ôv_î@Ì/E½ÏY?ÿ.ÐG«<?¤r(çTã\?±y¾\òt@T©p¨	@
°4–	Â?æ^Å󔷳¿Øuaµ|¤¿àÙàvoÉ¿ß@dtß¿äÜ&$p¿âF•Ew–AGNbll3FGL J0856.7-1105PMN J0856-1105?ïýð‾?0\A\O}?7@yL»Úë?0\A\O}?ïë¿¥-1Î?c®Å–ÉÔ?d@[?c®Å–ÉÔ?ïéoW¦°?hr4ë?f¨œ¨U?hr4ë?ïÑם­œÓ?^C× Y_?w1Äz?^C× Y_?ïúþY?Cx·šgÿÞ?G"]]?Cx·šgÿÞ?ï ï]_Ez?–¾é+ʀ?‡Ä(¤¿?–¾é+ʀ?ïӐú³?ƒ âT¿?vt·—óZ?ƒ âT¿?ïZßf¤Ç?€£:øF?"¤.Ö¹'?€£:øFAGN4FGL J0856.8+2056?ÏdÈõ…[R@BD™÷LÀ9úÑáÃôÀ<<FipÜâ@7"/M>@'q›MÏ?º á!§¼?w(ø¿n?âÏbcøM@H[¦™Ý6¿ïÜô‰u?ìýçՒï¿âå‰\4´=¿â•€/eH¿ÝÝkëáe
¿â\&$pAGNbll3FGL J0856.5+2057TXS 0853+211?ïüRÑ»/?0•DFx†?=oŠú­…?0•DFx†?ïóËI‹t?WpœË'[9?Xilù#'-?WpœË'[9?ïð¦¾Ài?dSäÖÉBÜ?^²"Uqlñ?dSäÖÉBÜ?ïê¿{Ì]?PE~¦" ?e@ñe÷g?PE~¦" ?ïòÀ ññ?T¨3ɵ?ZÀ-ݙ?T¨3ɵ?ïΞÜNŸö?xè"m†¡?x°'øLl¿?xè"m†¡?ïã;)²è?xÃb£ŠÊy?lÄÖvSJS?xÃb£ŠÊy?ï¯ù¥Ñhñ?t¥&?¯ÃR?"–‹ý¹§?t¥&?¯ÃRAGN4FGL J0856.8+8559?Ø<%{v@=(dŒq"À;c~h»«<À<¾¸‡›jT@·à™³Dæ@'ÉÜW"K?ÎÓw¾RŒ?À*ךOJ?î*Ö7¯™¶@Ň3:•¿ìøžï!‹?ãgc¼gú»?āBJR^¿çw5<滿àÆ7½¯l¿Ú¹9±ÊéAGNbcuNVSS J085740+860344?ïþ'ò·?Y'ìSÛ?/ÍS'9î?Y'ìSÛ?ïöÑ>\Ã6?Q!]\ÏQH?R]ƒFy"Ÿ?Q!]\ÏQH?ïíQ|ò}?c[wZ4•è?b®ƒ¼²«=?c[wZ4•è?ïóÍùXØ?>ûÆoó{`?Xd
"TÍ
?>ûÆoó{`?ïü6ðÌ[?:¢×ÑEú!?>OBs¹Í?:¢×ÑEú!?ïÏ5Ö.S?|È._j1?xeãÂÂ?|È._j1?ïØço1Þl?|úbmn©'?sŒH}¾5÷?|úbmn©'?ïÓ}-RH¢?d+ÊAV?vAithR¿?d+ÊAVAGN4FGL J0857.7+0137?æ=]ĉåÐ@<™;ʸÀ;8ž'7À<‹m{-È@…9C¬Å@tßÔŽ?Î.†¦!è2?Ëõ%Ü]Ž|?úPÞªDâˆ?ö¸Dý?ïðÓÊ¿Ç""FZ¿èˆóß`MH¿ÙeNëž¿ð?ïÿø¨ó©°AGNbllRX J0857.8+0135?ï®ëüÏF?…•è(*¾?"E̖äŽ?…•è(*¾?îæt–Þ[ô?¨·‰'jëì?¡˜¶Žª¤Å?¨·‰'jëì?îÓI²6ڙ?"îœÔ':è?¢ËdÙ"ºx?"îœÔ':è?ïhyLXY?"ã0-ȤÅ?ŸòðÔ½&Õ?"ã0-ȤÅ?ïŒ
'ÃD@?'¬aS ?Œü›Y}ÃÒ?'¬aS ?䂻è_5¬?ÑŒŠ£˜²?Öúˆ/A"¨?ÑŒŠ£˜²?펙Õöäp?¢@÷ZÙ¯"?³‹1Q$À?¢@÷ZÙ¯"?施"²"?¸gPuëý?Ò҄×À›¼?¸gPuëýAGN4FGL J0857.9-1949?ÖNʤ¨@0‡Ò"œ²SÀ9`ây|À<kc%iF@-_«·@'ãt®ÿ?¯©.Zêî?Ÿ¾E†®¹?죦-%Òø@6rÆÆù?ÖÙo]»¿ä¤øÝÌÏQ¿çH/^'\Ž¿åÐZ‹fÐï¿æ…bªð3¿ïÿ‹›ªAGNfsrq3FGL J0858.1-1951PKS 0855-19?ïýý0dCC? ô<6Ë£Ÿ?0}ºæ`ý? ô<6Ë£Ÿ?ïò)Œ&¥—?^A–T>t?[¬çU?q¸?^A–T>t?ïñ¾¯äÅÎ?JHX'?\'Ÿîü"A?JHX'?ïþÏäŒæ?ÙµäE²?.ó/:Ž?ÙµäE²?ïþ-ùÊ?!¾ÑÇë_?'ív0'?!¾ÑÇë_?ïµ^ýDŽ?Œ§+
Ûñê?'¨@®¢f†?Œ§+
Ûñê?ï犣\û?mâ‡ÖÄäs?hu\åg…?mâ‡ÖÄäs?ïûs\C?5Ñ´}¢Ï?B2nŽ¤?5Ñ´}¢ÏAGN4FGL J0858.1+1405?í¼ÎNõº@A.j¨ëF5À:¾ã²Â_ŒÀ<oy¼"€@:ªÆg­ä@y\ã/å¡?ÆŲýî?½Ç;¾G"ÿ?ð"X6ù@±øÀƄ3?îÍÑ–0¿Ï­ò';׿è¥8hýœ¿è®½>¿â%Á?ÐÐh¿ïÿý¡UûŠAGNssrq3C 212?ïû%6©.?:ðx»±î?Ck'{}N?:ðx»±î?ïâDv=Z?rŸi-Š?m»ügfö?rŸi-Š?ïÁ Ûq7?z[¯—G…×?/'Ec ²?z[¯—G…×?ïǐöÔ?anWt[?|7…[N?anWt[?ïù?Ë-K¤?IMº|•u?KÔ.2Ó?IMº|•u?ïz™kÌVÛ?"kåÕ}«?¬Ò†u$š?"kåÕ}«?ïoþµIšË?Œ>sðɞ?')Oín§?Œ>sðɞ?îG{ÜBÞ?–ߨÂbƒ?«ˆB@W¹?–ߨÂbƒAGN4FGL J0859.4+6218¿çpøiø[
@CDhۋ¬qÀ:ÀõÄ<ÛSÀ<±‡O:J@4·jºÞä@WdU/?½åœQ"×ì¿}æñˆTC?½ðÆQ2¢•@u3`œ˜?ìžÊÆbO€¿Þ—u;Ê¿èú'`åóå¿×µ£euP¿ç§ÛACl¿Þð?ãÅ·°AGNbll3FGL J0859.1+62191RXS J085930.5+621737?ïþÁÓÛm?.Ð?#âÏÙÞF?.Ð?ïö‹6Y­?R€žüÿøM?R铼Ö^?R€žüÿøM?ïø.sl•?B¢#k	D?OF3'ÈE?B¢#k	D?ïúŽð"s(?,kQgT%?EÄ<àEDº?,kQgT%?ïýÔùäTu?*"y/õ¶?1X0yNÌ?*"y/õ¶?ïÜð
êiÁ?sQˆÆ8f?q‡ú"j–?sQˆÆ8f?ïõ½`?¨?`@ärÃä?Uî……¯á?`@ärÃä?ïïu£ñp?LäóÙe?`Š[Õ;Ú?LäóÙeAGN4FGL J0859.4+8345¿îîxð{@>MÊ:KUiÀ<êäåÈFÀ=5ôÆ/@"˗‹!†¸?ö¾0'}ó?Õª• Õ`?юcpàÓ?÷ÄÉÉMì@ž}"D¿ïÿðÇô ?ïùªæÈ÷U¿ïÿoì÷å?ïþ=BUºó¿Ñ¼§›dõοáñ@ÅÂíAGNbll1RXS J085916.5+834450?ï÷ç_A¦`?r5mO?P1BªMÅ?r5mO?ïôq~>ìœ?X…ðËÖÁç?W'&Ç{?X…ðËÖÁç?ïvR/ïÿ?Œ•˜ŽŸ9?'.U±jú(?Œ•˜ŽŸ9?ïûF
ðw?9é\™²'M?BçÈ…Çž?9é\™²'M?ïïǼÓÁš?`–/¦?`8Bñ%ƒ?`–/¦?ïÌÕ¡ËK?tՓ''î?y•/‹¶K?tՓ''î?ï‹t¸c´/?‹òç"?nK?"ÑÜÄ 2?‹òç"?nK?ïéùïM]ß?cÁ©±ÖX'?fÖ^m?cÁ©±ÖX'AGN4FGL J0900.6-7408?ïªÔž—.À1úgèF¥×À:1Y³Ð|…À<7ä¼­šØ@~Ë?"@¢ùà0W?Şԁw
þ?ÉhÚÆ_ ?üö*ÿˆ
ü@	}Ð3´f?àbù"«ô¿ä~Áï#9¿ë¦°8Aí¿îg"¾Ái¿ÑAÿE¿ïü-""ÑAGNbcuAT20G J085959-741401?ïûœ–×¥÷?IðF)Õz?A¤\#6E?IðF)Õz?ïóL{r?^Lô`HÅ?YÉg'
=ƒ?^Lô`HÅ?琢èÑ»?YYFe?…Eˑ8w?YYFe?ïûÇ…?-ýɈu?@ãýx`ÃË?-ýɈu?ïüwÅ^nu?Bû¨iT?<AÓÊd*V?Bû¨iT?ïÔöµ\ p?{0œýç!?u"¥7ÒÀ/?{0œýç!?ï8`ع?•?ìhÄE²?ž8óöä Ç?•?ìhÄE²?ïÖÓQÝS"?h¡Òäv3?t–WFr?h¡Òäv3AGN4FGL J0900.7-1243¿Ö&
Žf"@5SÂCÜΣÀ:8èí"ÃqÀ<`ÎùͶØ@ßڃïŽ@"'A?ºh…¥pè?˜tŸ¡?ß"äRzv@VÞyzÐ?ïÿÞ§À£Ê¿Êši7Ñþe¿æÀŠt8¿â-%Òø_ù¿é-"BJ'k¿Ú&$"AGNbcuTXS 0858-125?ïýܟRÁ?$§ütFÖ?1æe—?$§ütFÖ?ïóƒòàª?]¥L£™è?XøÈy9&?]¥L£™è?ïä74t¦Æ?k &ã°õD?kÈËdݚ8?k &ã°õD?ïþñ"?ÈñíÕËÙ? ç"ñ´õ?ÈñíÕËÙ?ïüQnñƒ?:æ.¤ÇÓ3?=s"ㆩ{?:æ.¤ÇÓ3?ïÏ"?öüèE¾™?xr÷
Ô1?öüèE¾™?ïÎwJ?~ÙeÐ'ý?xÄ[‹Á¤?~ÙeÐ'ý?ïþ'Cð?u~Ň?.ÕAs'Ü?u~ŇAGN4FGL J0901.2+6742¿Þžh3"@B‹kü¨\«À:iTK±¯:À<cۖ"+œ@¥À$Ä!@rü¬Žhä?Ã_5'n·y?Âf‡s|O?üvѵ(@ ov°?ïõ8ü Ïï¿âçí_>~ì¿çÃPýsˆ¹¿ä4ÂI¼´¿ïÿ¤€RuÄ?ä‰áàÛ!¤AGNbll3FGL J0900.0+6754TXS 0856+679?ïúj'ˆcš?X#…^'Ñ?FUöSŠ®@?X#…^'Ñ?ïò›õ®1E?UË`Àçì?ZÈUI?UË`Àçì?ï㮜ú»â?c‡ö=8a?lQc5^¥‹?c‡ö=8a?ïËéfÐ2w?aŒmM>¯?zL¢å""?aŒmM>¯?ïëÐ9$*?d
Ìםú?d/ǼM{?d
Ìםú?ï·íI;ª?'µ{{ç! ?'­´7»g?'µ{{ç! ?量Ÿ§>?‡%¸8z¡°?†XÀÀÞ?‡%¸8z¡°?î‡?¡"z?''RäÉä?§ŒëÔ`?''RäÉäAGN4FGL J0901.4+4542?̊4e§˜@DªV"uÀ;É«¸€®À<ï[:¹9r@ù"D›?ü‹rX?á^$Ñq?ï÷ÝâsÓ@$ †å@í?³õ¿áën"cÔ¿ÁÞ/5L½ô?í_«–òm¿æwˆ,‰ËÆ¿ïÿԖũÃ?ç
ò¢IlAGNbllNVSS J090208+454433?ïáŠÂøHã?yy¾ZŠºU?nu=!Ô%.?yy¾ZŠºU?ï²Làņ?–X¼ÉcOŸ?ƒlú•?–X¼ÉcOŸ?î³ï
òå?˜ãÂ}U¥«?¯"Á Ñ©?˜ãÂ}U¥«?íÌmn˜d?žþ jªT
?±œ"‹ªÓ?žþ jªT
?îí8°þ?¥¬/¿Ï?¡/¼q'?¥¬/¿Ï?îK>5€ü{?¸!À`Ö?«L¨ÌO?¸!À`Ö?ë¸	Ç)?¬ƒ(ªH\s?ÃÍØã[…?¬ƒ(ªH\s?éO¨(º?»zô#9&N?˲Ý_]?»zô#9&NAGN4FGL J0901.5+6711¿ì~V[¯¼@B¥Ÿ<pÊÀ;>Iç«À<Ÿ.X•@ 'è(ó¿*@´{'G–?ÂÝ`t#"¿…ùN'fn–?ÅúöÖ¶…Ž@æ"Ïíú?î'"2wL?Ö"D"™³¿äx7ÿ˧´¿àõ½ò>v]¿Õ¸"þ<[¿Øæþ§:l
AGNbcu1RXS J090140.8+671158?ïýÓ;¶²?"›'m"l?1g÷Œµò?"›'m"l?ïö(¹7¤?R46J5I‹?S®M"7ö?R46J5I‹?ïöbºà;??TѱO!2 ?S:‰úÑS+?TѱO!2 ?ïõŸLƒ^?9­PtX?UâÀþ…%?9­PtX?ïüœBì8Î?1©æ²	è?;ꉴáú?1©æ²	è?ïÔ.ø³Qô?z'jˆžòa?uèƒÅCå?z'jˆžòa?ï÷"²:-?bæD±ž1?Qõº(Æ ?bæD±ž1?ïÒÞx)²?eö#\¢T–?vÃá.—7?eö#\¢T–AGN4FGL J0902.4+6440?éÆæY÷ÔI@CàÁvWuÀ;A&"Ï:À<ÂFÊ¿¬S@ǯ½ó@)@ç*໗?Å°'åøý¿ OáGÎ?ÖùDåè¨@ïƃ°¿âëE=¡Ì¿ë'} <5¿Õ1e¾àÆ¿ã¸É_¯èæ¿Ü¬W¿ïü­/x"AGNbcuGB6 J0902+6444?ïü²Hš¬?1…³ÕÚS?:m»ÆÀ""?1…³ÕÚS?ïõ­¢vHB?UT
dL »?T¤º»y|'?UT
dL »?ïÚD‡C€³?y~Äõž˜S?rݼf~¶S?y~Äõž˜S?ïûß/éŽ?%ñÊ	Zf
?@ƒ·¬u™?%ñÊ	Zf
?ïú ?ïð??¢Öá<x¡?G2hSè??¢Öá<x¡?ïÓ#hq?|"6*ûÖw?vnL$Ø?|"6*ûÖw?ïÉã3¬?ƒìç®K¼?{f‹×d'?ƒìç®K¼?ïéÓ_ÛTF?W'º–a?f,ŸêòIÚ?W'º–aAGN4FGL J0902.4+2051?éUSî@BàûC؜åÀ8ë+•°À<út¥ÄJ@𗏩*Ü@ã`dÄ¥·?§ŠI€¸³L? Ä©H¹,?ö;ßßÏ@hGn~Ð¿Ò<Àåä¿à5Úã1¿âIšHB‡¿âTä(3$ð¿àF4—·AJ¿éE‡=÷\mAGNbll3FGL J0902.4+2050NVSS J090226+205045?ïþoC|#	?,Gçì?)ÇïøŒ?,Gçì?ïöE@ÜË?Wd"w;%f?SuŒÚü?Wd"w;%f?ïöŠ¡?\:¢ÕåË?Råã!·…Ÿ?\:¢ÕåË?ïý|Ù?$׊߾™­?4N²ÿ-?$׊߾™­?ïþ#8>¸?"q‹ÚP…_?-Ì~…HD?"q‹ÚP…_?ïØÀurë&?vz'W?sŸÅ9{è×?vz'W?ïõ Ä8Ý?eJ˜Á3½?T¾wZ²Ž?eJ˜Á3½?ïûy`>.9?6¥AÀ¯%$?BxÏ??6¥AÀ¯%$AGN4FGL J0902.5-4801?»6í+UÝò¿îÃ"N®ºÀ9 ìt2À:ÞÿÕ8@›ýèx¤×@Q<\§¡?Îãî<Cñ?Üj¹œÄFk@Nªß<;?úi·¬T1[?íD8¿HB¿å¯m@u;¿çÐÓDM¸¿ìŽæbJ"
¿ïÓ±B'±v?Æ4Ü5JAGNbcuPMN J0903-4805?ÞYz‹"µ?ÒQ%èÙ"?àÓBº16%?ÒQ%èÙ"?Ð9Œé:Ÿ?ƳÀè¤)ý?çãx¹‹b°?ƳÀè¤)ý?äþÃB=ï?µÇµ"z`?Öy{…Ì!?µÇµ"z`?Õc£`öB›?±ÏQQXœ?åN.O"Þ³?±ÏQQXœ?àÌWÒ­j?Ò̬tb?ÞgPZ¥+ã?Ò̬tb?'íqJ?šâ.içþ–?ïp"wƶ?šâ.içþ–?ÒF	4î0?¶Vdyqóó?æõÜûeˆè?¶Vdyqóó?žÿpIOe?qÙÙ'?ïÀÂd%'?qÙÙ'MIXED4FGL J0903.1+4652¿ï(tJL â@DÉ}ke©¨À9ǽWäÃdÀ<{¬h©6Æ@òS™Z. @üc®%AÙ?¬¸9lÞ$¹¿¤€ýbäC?ö‹‹Ÿe@zêéz¿ÚÙaE?OK¿åÍ:°ÕöA¿ç0[b&eÅ¿åtáTù׿ÞFãÿ™RÍ¿ìàÁvWu2AGNfsrq3FGL J0903.1+4649S4 0859+47?ïþc¿†×å?Ñí4_Ç?)Ä
90?Ñí4_Ç?ï÷aź+?Q.‰ô·œ?Qï<"	Å?Q.‰ô·œ?ïòfLð¢?cÕÐKC_¥?[3fµÛ³?cÕÐKC_¥?ïó¾É¢?CŽ×ò8å?Yî'6øûÚ?CŽ×ò8å?ïýwoÖ°.?+'HáÎ8k?4D'›¬?+'HáÎ8k?ïÔc@än!?uõo,¯r¶?uÎ_z‹Ò?uõo,¯r¶?ïì羄yf?p#±Zâkô?cA…%'<?p#±Zâkô?ï·L/Xˆ,?sÍC¦5Ò?',ô7*÷?sÍC¦5ÒAGN4FGL J0904.0+2724¿æUÌ",ûŒ@C÷Ä"`À:E®†¨YÀ<|Å<µ'ô@ïIp6t@~*Ã") ?Á—ø¯©¦W?ÆO¬e¤®?ÿ¿ôw5Áƒ@	¹H~?Æ]B Ç¿ç§"™2¿êß"²¿ê§}½›¢¿ïÿÞr¾"¿é´á¾ÌY
AGNbcuB2 0900+27?ïú ó*.¨?FÊŠ—Ø?E|4ˆ©¼?FÊŠ—Ø?ïñÅ`Fè?^%ˆ•ÝAÐ?]ætÁ'y?^%ˆ•ÝAÐ?ïÞxµ.ì?_yΫÿ·®?pÃ¥G&ùø?_yΫÿ·®?ïØJÛE‹?\{º:Â×R?söÚ¦Jö'?\{º:Â×R?ïöM'Gv?S$&Ü}æÖ?Sdû`•¸U?S$&Ü}æÖ?ïÀ§3q‡?~읯IJt?¬fw°›?~읯IJt?ï Ô)*½?…ÇTÎõ'4?‡Êõ¾$ì³?…ÇTÎõ'4?îèx¬[Š?ŠÄ>¢–Ý?¡xu9kp6?ŠÄ>¢–ÝAGN4FGL J0904.5-3513¿Æ̧ç«@<Ù|ÞwðÀ9cЗ\¨À;Ô¯ÂÐʈ@'º.9¤<@¡&cAø?¹VÈ8¾b|?Ä@l³sà@#xà¼mÚ@.="‡¿Ì
#)$çk¿çw9ó@ÔÜ¿ãঋ(¿ë2O¨´¿¿ëÛÞ´UÞ?¤@ª; gAGNbcu3FGL J0904.8-3516NVSS J090442-351423?ï±ô"•ðÜ?©ŽMP}?ƒ'÷^KZá?©ŽMP}?ïå·¤?xN"È}?j=I,³Ù?xN"È}?ˆ)ÀÕ?†"¿Psœ?‰Ü]Ô?†"¿Psœ?ïý僧êÀ?±/¹«?0Óãâïc•?±/¹«?ïìÀóÃå?`¶ÄâR=?c?à'à?`¶ÄâR=?ï?=?«Š´®°Èƒ?xDŸÇO?«Š´®°Èƒ?îSÃ	CI? s–FE7+?ªÃÏløv? s–FE7+?ïö³Ÿ‡Î?FBøh‡á½?Rޘðm?FBøh‡á½AGN4FGL J0904.6+4238¿íc3'¹æ@Dø<÷TÀ:Ÿú D®†À<¨¦tsoc@tTc¯|Û@ôóg°?Ä©À˜¶ð˜?ÁǶb}#?úOSû)×?ùA˜‹Ò† ?í@֟^'¿åIÁêñ{¿âpŒû%¥¬¿â}5€V¿äpŽ•·¿ïÿï¿@PAGNfsrq3FGL J0904.3+42404C +42.28?ï÷Ü.ƒdé?CÐ]õ"ªf?PG¢ºŠÖ?CÐ]õ"ªf?ï¢Þ7"}?ˆl‹íª*?‡Hr
"M>?ˆl‹íª*?ïÞòõç‰x?l
³¶Ü?p†"êJ?l
³¶Ü?sY
?ƒHÚÀø¦?¥&_œ:S?ƒHÚÀø¦?ïÇ]kYÚ?{j)_Ž÷¥?|QJm0ñ?{j)_Ž÷¥?íZÞ´ð{í?·4	0mk?µ)
Z¡â?·4	0mk?ï \4€³?‰:Êæ'%?‡ú(òßÓ\?‰:Êæ'%?é×Kðˆ-?©üˆJµ'?Ëè¢Ð=ßM?©üˆJµ'AGN4FGL J0904.9-5734?î'²¨xÀ$«>݋aÀ7ÉÜ_çÇ$À;IŠ]ÜT@©b"@Úºp©¶?˜#yç;?¥´t€b0@
6lmçd(@"›æ¥ç¿xÇ!€òól¿â$Ÿä6v¿äFÿ=T<¿ãw÷*|«¿ælŒñ«¿áÛ~ AiAGNbcu3FGL J0904.8-5734PKS 0903-57?ï7WP…Ù?¸c10W>?™ê6ºÞ?¸c10W>?ïðý·?6?q¤xŸ•ÞV?_Òó3Ý?q¤xŸ•ÞV?ïâ鉛õ"?sr¶
x?mv-«à?sr¶
x?ïÿÀ-hT8>õ3µ'2Þd>ÿég`Ö8>õ3µ'2Þd?ïþ®Ìã?(auª,Lr?.¥÷[²Å?(auª,Lr?ïŒ"5ùÙ?¢©Ì£¤bà?Œþšïíª?¢©Ì£¤bà?ïЯgX¡#?}ÒâeèHž?w¨L7'¢ƒ?}ÒâeèHž?ïÿ¤Û—?
¡UÎ9Úî?É$'ãD?
¡UÎ9ÚîAGN4FGL J0905.6+1358?ÆÓá¥2:@AûÚ¾'œÀ9PvÄ À;Ì(Hôe˜@:grÕàr?ùv÷xr¥?²‡›À:m9?Àk.¢)àú@ll—ØÏ:@
õÁòSD ¿Ú½'Æf>¿º{Ýñã1¾¿Óžœ"_ü?¿Ñƒ%Nn"¿àäëa¸VÉ¿ànÀY!AGNbll3FGL J0905.5+1358MG1 J090534+1358?ïû8áÚ`??h–þNå?Cw¤GË=??h–þNå?ïéÛ:p5¿?f*ŽPê™?f$ŕI ?f*ŽPê™?ïÙ""6-0?s€Ê¤9³?snîƬØ'?s€Ê¤9³?ïÖñÒQ?Uqe(ñ?tû†øšïz?Uqe(ñ?ï멖^H,?b_b¶5‹?dViÁT;ž?b_b¶5‹?ð[Oå?ŸïçÍI¹?ˆÛÃÞÝ2°?ŸïçÍI¹?ïئ&3µ?€³HãÊó?sü¬ë†Mn?€³HãÊó?ïRôê"H)?|±˜6î?•¡b½nÈÑ?|±˜6îAGN4FGL J0906.2-1707?îïT«°·@3¾G'ܾÀ;"æ>ÚÀ<l»êý9@ x–†>Èé?þ0M:Ev,?ÑÕn'€ñ?È;™¼)<?øääÖ®ÍÞ@4ô‰)^ô?ïÅì=«\:?̵FÞ¶¯)¿£O.D³Å¿Ú>Ù#ó$O¿àœ¨AÓ	'¿ïòË.g˜AGNbcuCRATES J0906-1706?ïù%Ôó.?@è"[5¨?KÇh–5Æ¿?@è"[5¨?ïՍà 5·?uøZŸB¯?u9¤æd[?uøZŸB¯?ïڈNvä?l 	.U¿?r»ýņ¾?l 	.U¿?ï™	Iæå
?jÅñ5ÿ?‰½­u°Ñ?jÅñ5ÿ?ïõžäBpy?P×f'Øý¬?TÂ7žÚýŽ?P×f'Øý¬?ïjŒõ¶è?›\•¹,Š?'®aD?›\•¹,Š?ï¦Öáx«b?"¤`ÌΙ?†JGšõïn?"¤`ÌΙ?îy©"ÚV?'î;¿J"?¨f%jFœ?'î;¿J"AGN4FGL J0906.3-0905?í'J^Y7æ@8'sÕº²À9óÿò"³À<Qäþú2@]oqÒÖ@^쿱[W?¹*³Éƈ?´sßrkØ?ûåCÃC@‡-ã"ã?ï;ái\æ?¦½nú£¿ÝÞa_@'Q¿âØ)Âq)8¿ç!½T‰Å¿áŽýÉÄڐAGNbll3FGL J0906.3-0906PMN J0906-0905?ïþ‹Š¦üG? 6f@?'GV**R? 6f@?ïõœæÄß\?XSHâ%Z?TÆ2÷r–Œ?XSHâ%Z?ïïh+ž¥ƒ?f(ŒÏNaÙ?`—Ô"!­?f(ŒÏNaÙ?ïü^èãY?'.‰ Ÿ?=ðÜlX?'.‰ Ÿ?ïþf…Δ+?!PZbƒw(?)—¡•é@?!PZbƒw(?ï֕^#T?vDIT¼ê?tµsï*å›?vDIT¼ê?ïé^³'?tEôÎ@Ö?f¡M6Ñb³?tEôÎ@Ö?ïù²µŽ0Ÿ?8ÃÅ¿!{?I5*2þÃ?8ÃÅ¿!{AGN4FGL J0906.7+4950?èíToÿþd@Dõn?x»ÔÀ;•X'ßBÀ<ÚpΟ4ä@JÏß%ë@RÈqz?Ì\K‹*¿Kñßő´?ÐØV"¡jž@*6jX‹?ïýùà¬'¼?ÈÅq¤2#ê¿ìâ?z¿¿®UÙa–Ú¿é×»]Ž¦v¿ïåj‰
ÖAGNfsrq87GB 090322.8+500444?ïý»ÂŽZv?=I
¾'dQ?2!í¬Tñ[?=I
¾'dQ?ï÷™X<h?Q뜉Ρi?QôÍ{'/*?Q뜉Ρi?ï©M¦Ñæg?"ÙÃÆ·áŽ?…¬–:XZN?"ÙÃÆ·áŽ?ïúÌ5Å£?/nKÙQº?DÏ ¨Zb?/nKÙQº?ïúÃV<³Ì?Hp£ƒ?Dò¦
%Ö?Hp£ƒ?ïÕ8èÒ+?w4''¡¾?ucÿ¥n‰?w4''¡¾?ïgiޔ?'/ÑÝgV?"܋·>?'/ÑÝgV?ïê&'7?Xõ/ÕKD¤?eÙêèqÊ?Xõ/ÕKD¤AGN4FGL J0908.9+2311¿ïf©EšO2@Cô$_ZÙjÀ9ܺã–<îÀ<%˜°eù@ çW˜BV'?û
RH¢0A?¼Âs,lã?»óÈd2Z@M€ÿnàˆ@[,þåÑ?ïÀ¦]ø-Ï¿ãIJh!R¿áŒ…0aÈ¿Ôð¤ÃCa¿Î-)ÙÃ*b¿ãö9þ(kAGNbll3FGL J0909.0+2310RX J0908.9+2311?ïþxX"Î.?˜#žl?(z€›˜ïz?˜#žl?ïòؾXÑä?X;Òu•0?ZNƒ"f·?X;Òu•0?ïù^2w?;"šS†³Ô?Kû»x+?;"šS†³Ô?ïçû÷ݜ©?Jʐù›Ì.?hZ¼îï?Jʐù›Ì.?ïýEââ?)•/Õ©Ó}?5Ñã^÷î¢?)•/Õ©Ó}?ïé9D?Œš"Êh)?~|+YÕöK?Œš"Êh)?ïñjžÉ?gWF¾KnÚ?]Ï+@ßdó?gWF¾KnÚ?ﯴ€<n?q»Í¨Ç¯?"ßñ	ʇ?q»Í¨Ç¯AGN4FGL J0909.1+0121¿í©.·ùV@>í/IŒ;À8SÓíçÐÀ;¥­'ž"•@Á˜€iò¸@ì´^@ý÷?žT©œéQµ?¹_¿p@
¿ó v@ð8æP?î‹#Ÿ—_ƒ¿ã¯Þø¿è>þ#†î¿å¼Ù¿úVs¿êìÔÿ÷«¿ïù0¾
í)AGNfsrq3FGL J0909.1+0121PKS 0906+01?ïñ»îûmA?YU/¶я?\ˆ":ŸÞŒ?YU/¶я?ïóŠ,Ozx?`k'•áuž?X맶A_ç?`k'•áuž?ï†o™|$?ŒP?—÷VY?Žz$R#&?ŒP?—÷VY?ïüÚËVïÀ?*pÊo@a?9)¥"FNç?*pÊo@a?ïõ€Sç!§?R©2µÕ$?TÿXÿƒ?R©2µÕ$?ïÏ.܌]q?Ñâ#3Ö?xh'ÉŸ{p?Ñâ#3Ö?ïTq˜þx?"8ô{-?•qÌýÈbó?"8ô{-?ïõý4·º?FÅÏ(Ûå?T׆kü?FÅÏ(ÛåAGN4FGL J0909.6+0159¿â·Š(kÅ@?\œÃŤÀ9DkHMwÀ;ëÛd?D¹@"ØБ(@ZÜ
²p?·` SÇþ?¿äq.@…@Õ"Ü£Ú@e骩}¿ë"ÎÁnŸÆ¿ÜQj€ÒMj¿ß;t€¿àW1	G|¿çDP'èË¿èx¼_eóAGNbll3FGL J0909.6+0157PKS 0907+022?ïýBɱÂä?0	búvK€?5é´e…n?0	búvK€?ïäd'5½Á?rŸØ_–€B?k›Øò¶ï?rŸØ_–€B?ïñpcH?\§B›NY8?]9Øq!R?\§B›NY8?ï‰bɘ?tàIʂÿQ?¾§Q/uù?tàIʂÿQ?ïîR–ÙSv?`èRî7±?a­imyŽ?`èRî7±?ï§Ó¥rڂ?Š©%Ñì^r?†£I_‰?Š©%Ñì^r?]	gÕ?\«Iâs?Š_h¯çšÌ?\«Iâs?í‹rGxÃ? CA6?Òà?³¤mŃÁç? CA6?ÒàAGN4FGL J0909.7-0230?îŠåæh@<þrÚ/­À8'æ:\aÀ;ƽÀÀO@#êç¿í@@Ñå:Ü?£+w'(ãÏ?¹ºÙ…AóÀ@mmÁ¤{@K¸»÷¿ÁæƒA¾fX¿ÞOX,翗¿äÆÄ	¯¬+¿ãò<'Î{¿ëùÍNY¿Ù#''%ÎAGNfsrq3FGL J0909.8-0229PKS 0907-023?ïö˜Þ¼A?KûŒX`I?RÎB/‡Ò|?KûŒX`I?ïî•ŒwP?gššÈ[?aíj00X'?gššÈ[?ï=׌¡í?"3ÅcÓ¸D?˜Eo1û¡?"3ÅcÓ¸D?ïïlh¢Å?GǛéa?`"—¯@?GǛéa?ïò>£v3°?TW–áv±œ?['¸ê]O"?TW–áv±œ?ïµ`zî^?‡†xP_"?'§þecðŠ?‡†xP_"?ïD¼~å§ÿ?"yZ•pò?—hp%Î#?"yZ•pò?療Û§S?tÓʟxd@?†›¾ÇWk?tÓʟxd@AGN4FGL J0909.7+3104?ìU¯kN5@DõË£!hÀ;PKúˆÈÀ<ÎañŒŸ¶@ 7‡bàJ?ýñk—þŽç?Ë£ƒè­S
?·ÑêK¸»?ì[›Â=Ҟ?ýž…´Š`Â?åÇà~ÛRL¿Ñ›Dß­úû?ÊÛÿ…0Öâ¿àxzЀ¶t¿é6añŒŸ¶?Ä]Ý@bp¸AGNbllB2 0906+31?ïûå¹­¶1?6÷¾Y¨]«?@i x¨^?6÷¾Y¨]«?ïìÛòì?c‹Wd¨e?c$(ìñ ?c‹Wd¨e?ïÕ¨ËæÙ?qcâêy½¨?u+š¿—L?qcâêy½¨?ï®Z›Ï?f†HLS¤p?"yšœ@?f†HLS¤p?ïù*-&?BœÁ-šg\?KWKmÜ¡ó?BœÁ-šg\?ﻤúÜæ²?‡&N2ù€?ÁJÖš?‡&N2ù€?ï']º42¦?‰æ£48pÿ?‹¨'h¤'v?‰æ£48pÿ?îíµq€9»?‡
¿÷|MÙ?¡$¨èØKO?‡
¿÷|MÙAGN4FGL J0910.6+3329¿ëËÕEí(@E;\B 6À8܈'=À;ØÆï=:@¨Xx4?þn­È$Ç`?ªˆ͝‹?§yê&Ï͈@ì6Kìh@,ñê­Ø?ïõ@YŠ?Œ²QUø¿áS£ìó¿Ù
µà¢Á¿âêÑÀ&¡*¿Üj5"_õAGNbll3FGL J0910.5+3329Ton 1015?ïþ9¹¯Ë? $iØ!­t?,hmoÉ¥? $iØ!­t?ïïè}?cBƞì\
?`ñ꺲½?cBƞì\
?ïæeû[?vݑ9§'B?išL7µ}?vݑ9§'B?ï;µ~ ?{ŽŠlµ?±Äï+ô?{ŽŠlµ?ïú˜n?@ÍN­4ýP?EžE-Â?@ÍN­4ýP?ïȕÏëû?{™‰œ|?{µjJò¦?{™‰œ|?ïâþÞ¨þx?x_±þJf?m!]àÀQ?x_±þJf?î¤MÛ2É´?–·CÄ=¼?¥»"K÷}º?–·CÄ=¼AGN4FGL J0910.6+2247¿åWj"¥Ž@D;`(^ÄÀ:È­ƒ[jÀ<£_ëøâ@Fá'+¼@Œ—£TY?·à…;h¶Î?ÅlÉKR@/–@HÅl@ÜD!×?ÁâIá n¿Ñõª§&¿ãTגùlh¿ã·#240¿î0(QWáh¿ï骝i2AGNfsrq3FGL J0910.9+2248TXS 0907+230?ïìÇ^Mé?a]9äI¸}?c8¡ò¯¡?a]9äI¸}?ïö"f"v¯?Rs.0?RÙ2ŽÛ#?Rs.0?ï)²A
ïà?'Ù×êe£™?šÉ·å!;ì?'Ù×êe£™?ïüÿ:ïPl?#$.naŒT?8&Ðû·?#$.naŒT?ïÛCúoŒ?j'JªoÁ?r^½;3¯?j'JªoÁ?ïÔÖ¦üj?z{¹÷j°?uóÁr÷?z{¹÷j°?íúGV3q?¢W-²lƒŸ?°/ýÅNdx?¢W-²lƒŸ?ï÷ï¯óµ?@8dO†"þ?P  s¯*Q?@8dO†"þAGN4FGL J0910.8+3859?À¡H(ÂR@EáŸÂ¨‡À:Céœç+ôÀ<‰>xá"-@1o¦Öîå?þ#êÛ«Œá?½R'KÕÁ?º<kÁ:d?ÿ	9d¥œ@
PÌG@Ü>?ïµ{™>¿à6]õ~œ¾¿ázd ¯…¿Ó>.#~à0¿æegʵ¿åšQ_™¿AGNbll3FGL J0910.7+3858FBQS J091052.0+390202?ïþô¡Êb?_`qÞ±? µåÊel[?_`qÞ±?ïõ»º<²?Wwmuû?TˆŒX;°?Wwmuû?ïù[XýX?S¢ÊKdk³?Iʓ8,ª?S¢ÊKdk³?ïõBwÒR%?8¨2ÖÚ%?U{ÑëUà?8¨2ÖÚ%?ïþÁ{'NÇ?C§'3¾?#èF¯>?C§'3¾?ïÖõSÃe_?tQ!wøHÌ?t…Vïø¿?tQ!wøHÌ?ïøç	D?g»ÊLéƒ?O´ñ–û†ñ?g»ÊLéƒ?ï蓔iPs?Q€6'YGU?glkÁJ´Ã?Q€6'YGUAGN4FGL J0911.0-5047?¯'L²¿üð¾'dÀ9v,:ñm–À:åÉêpL@F\…¼íÝ@Œã›EkD?ÃÄxÖ*š?¥
$:qì?æìË:%•¼@s]Å­õ?îoÚê¿äÍ]"̃¿êL!@Âgï¿æ÷ ÈÍcÌ¿ÞMŸ½~ü¿ïÿâ¾÷!AGNbcu2FGL J0910.4-5050AT20G J091058-504807?ïù |Þ^?XIüX»ç?K÷}ª«Av?XIüX»ç?ïìKhfÏK?s‹•ÔZÿ?c´—°Ž
V?s‹•ÔZÿ?ïðzs[?—š:"«'"?áð³LlA?—š:"«'"?ïúŠÊÂË?0ʤÎ?EÔ×j!?0ʤÎ?ïß7²ìl?v:啮Æ?pd&•Ÿõ¸?v:啮Æ?-Ð?¢ž]©¢|÷?Òú{k7/?¢ž]©¢|÷?îÏ(=¥–Â?›ãy˜†Û?£
|(:Há?›ãy˜†Û?ïÖ­ag?hˆ&I©¸ê?t©~ZK?Œ?hˆ&I©¸êAGN4FGL J0911.7+3349¿ã…x;"Åc@E_0"'À:}7褚À<FÞ˜¯@1{™>@…¼‡Û+4?¿Žù£?ˆ™õ'œWî?ˏà³3ž"@Gò[§›?ÅïšØL¿é,*?ï"2¿ã®"&±¿ãhpa'ëO¿áRG•ÀÇ¿è‹Å .AGNbll3FGL J0911.8+3351MG2 J091151+3349?ïúD)Ùõ?8¼Ç­ÜI?FïWÒÖýT?8¼Ç­ÜI?ïõ°PóÁ?[dÓ	lT?UòŸbÎh?[dÓ	lT?ïôC­:–?SòïÜQf?Wx¥ÐÃ?SòïÜQf?ïð¥û/iX?BC"¹n
?^´	ã%Ð.?BC"¹n
?ïît&dæ?Tâá‰	åð?a‹ÙŠ›ßû?Tâá‰	åð?ïÔ󯺘B?sΆD'ú?u†(8±^÷?sΆD'ú?ïô]¤Ã:Ê?iE€úÓ¦Ÿ?WD¶POô?iE€úÓ¦Ÿ?ï¹7}´zŠ?kÝs¬«µG?² ¢¯'V?kÝs¬«µGAGN4FGL J0912.2+4127¿ÕÇö…5ù@E«ž¾œˆaÀ9ÍÆÇÐÀ<cJw—@¼³äsˆ@\±×?®žsóí£?¦-4@¤_ñ?ñäB"ßÎ1@€"[ï¿ì¿ÚÆÁ—"\¿âµŸSí½Þ¿èܦÿ³©æ¿ãµZTà,%¿â븮㮿ïÿAÿ~ÐÀAGNfsrq3FGL J0912.2+4126B3 0908+416B?ïþ©è—Á??²>[
?%a€îeðh??²>[
?ï÷+‰àWÞ?Xdü–Úp¦?Q¨ìœÅ£Ü?Xdü–Úp¦?ïó6á¾v?`Å#ꤦÎ?Yý'GÃT?`Å#ꤦÎ?ïÿãÄ^'>á_êƒ~è>ì;°cÚ$)>á_êƒ~è?ïÿQ:Éï<?
hM.÷D?ئúÙ?
hM.÷D?ïÚ®Š™Ê?t[œõuä?r¨ºï3ºÒ?t[œõuä?ïñ™	s=²?dB·¡HºÜ?\ÍìêÉìÙ?dB·¡HºÜ?ïÿÙ®Kq1>ìÐJ6Ôæ†>ó(ºS	|ª>ìÐJ6Ôæ†AGN4FGL J0912.2-2751¿íÝ:in"Ä@+×ß°Õ À:w©"ÉÀ<´9Xb@(½Ã@Ë—¦zS?ź†c±Ö&?ÓZ]-W§@
"Á{_ò¯?ýæϧóyŠ¿£ÝëœàdÉ¿Ý»÷<Œù"¿è_}¾ò™¿êL'ÅA¾¿æʳ¸(ÐÚ¿ïüƒ]œ"AGNbcu3FGL J0912.6-2757PMN J0912-2752?ïR+{+?"™ƒdÈm?•ºöqb£?"™ƒdÈm?çُ´¤ž?ÇÎF²Êu¸?ÐLà–¶ÃÕ?ÇÎF²Êu¸?îR‰sî?—FÕsܽþ?¦ú×k%+?—FÕsܽþ?믈óü^?ŸŠ¶«6õÁ?ÁAÜ0‡û?ŸŠ¶«6õÁ?îĚ=Z?®8EhUY?®Ó¶Zvld?®8EhUY?Ã/1ÒyÏ?Çt±ô•yà?ë4?3‹aŒ?Çt±ô•yà?çµ@ê?µKÒSƒç?Ñô•~+ÿã?µKÒSƒç?ʛëÑ'ƒ?³ÓGÊ Ì?éY ¶?³ÓGÊ ÌMIXED4FGL J0912.2+2800¿ë0ƒïŸpÚ@Dìä¸{ÜðÀ;REå"TÀ<¸é_ªŠƒ@!þfUõU¿µt'ÞÛ?æ$ãåF?ïÿÿÊPË@Dʄóð'@Ô«-•º¿ïýH_ë""?ïÿå"m/®¿ébP¢Yܕ¿álpk¢æ?âKYÎy¿åÍ+Í
dmAGNbll3FGL J0912.4+2800RX J0912.2+2759?îÿ÷q'?Ç×Jlµ¶?®Ð2qÜ?Ç×Jlµ¶?ïóa¹Ä?`ÿ}—d?Xå<€î?`ÿ}—d?íÙ¦O¬Þ?£R!Í£ø?±1êÍ¥'?£R!Í£ø?ïþhZ?$™9lµ¨?)~_&Ë¿@?$™9lµ¨?ïî‰FKz?˜šüÉiÁ?ˆ"] ®±?˜šüÉiÁ?ïÍEúÏÙ5?€+}数?y]¥ÑÕ-?€+}数?î¿êóö©·?šð…á`?¤PÂM2‡?šð…á`?ïþ8>#Àé?6ÍÍ£R
?,|ÄÛ;U?6ÍÍ£R
AGN4FGL J0912.5+1556?ï÷š«(@C#,¾¤ëÝÀ:™&dî—"À<uÄsa÷@!%³fm?ý§8ô=T?·—•á|Ý¿«¢%¯<4?ó$ہ›v@½íc›/ò?âúw_²íþ¿èSľ
'*¿Ó˜Í¡ˆü=¿ÝPô¤­¿èæló"
?àã"C÷¦•AGNbll3FGL J0912.7+1556RX J0912.5+1555?ïûOnÓr?BœŠ`bp;?BÂE)4	ö?BœŠ`bp;?ïô:¢Æǃ?WÎ&ÿGB:?WŠºKõZ¸?WÎ&ÿGB:?ïå¶Ùy7?p¥®zÒ.6?jI&eøˆä?p¥®zÒ.6?ïêÅ\Ú»<?N¤¯?>6é?e:£(t8?N¤¯?>6é?ïí¦(ô?`֕Jˆs?bãY›ò£B?`֕Jˆs?ïÄCj=?"Üó}¿7?}ÞJåⶄ?"Üó}¿7?ïÁØ= ûV?…<'e¯
H?ᏼê?…<'e¯
H?爵Î{'a?r©ËngŒ?…XLrIs'?r©ËngŒAGN4FGL J0912.9-2102¿È;…|¬#	@2|!ïAÀ9.qÊG·OÀ;à{.t‡'@ @É1aÌÏ?ý‹ÞÅó"¸?­ÐÂ¥¬wm?ŽÈfƒ4C?ဦÿÝo@Ÿ°É6¿ÜÛ@­ð¿åŠÉ>$(¿Ùeåvø…¿Ü=Ì4!¿âø?Â7È¿¹U@Ï(AGNbll3FGL J0912.9-2104MRC 0910-208?ïü¢Ðƒ6?0ŽÞõª­?:é€ÿä?0ŽÞõª­?ïòþ
¡3?[Ú~â™GÑ?[ôëv?[Ú~â™GÑ?ïò®a'Z?`B#¿¹p$?Z£þÏÍo?`B#¿¹p$?ïñɆ?N`¬=öÃ@?]õð4ƒš?N`¬=öÃ@?ïööá8·?KŽ{A­
?R>]Á Ñ?KŽ{A­
?ï¸G‰x܂?ˆJ¾¹:~?î¯ßEf?ˆJ¾¹:~?ïâÙébQ%?y;Xïxÿá?m&À
òw?y;Xïxÿá?ïۚ>žåù?ddu;?r2àœŸGØ?ddu;AGN4FGL J0913.3+8133?âíç•Gr@?ʝ@îÙÀ;qøòŅÀ<öŽhãï(@!¿ì÷åK?÷ìˆÚ.µ?Íßa$FE?ÅgY«m´?ûB=ú	F@Sx]3â±?ìäâ½ÏÙÈ?ì6«Ô.Á¿ÚÙ=—À|¿Úͬ;ç%?µ‡Kä/¿ÒÀ>ÉêDAGNbll1RXS J091324.6+813318?ïþÓ<'?f¿ðÓJ?"Ì:ê`0?f¿ðÓJ?ïõ™Ñ'œd?U,٦Ƿ?TÌ\|'(µ?U,٦Ƿ?ïìb¿<ìE?l}h™ó	æ?cA;?l}h™ó	æ?ïûO´¼r?1%mwWz?BÁ/{l?1%mwWz?ïþ…þÖW?#©V/¤u?'®TÀi	?#©V/¤u?ïÒ1%;ù«?~€ƒFf®Å?vçmG66|?~€ƒFf®Å?ïÕО­f?€#˜a'dŸ?uñži'?€#˜a'dŸ?ïò«CìÆ?SãµH®?Z©x{f#³?SãµH®AGN4FGL J0914.1-0202?êÃD''@>-inX£/À:è½±¦×À<[íâÇ
@Á_»ýF½@ûÜA´Ö6?Ã&¥]Œù¿§I#4{S?ä!7Ì¿a?þØ^€¾×A?ïù%P¡F¿ÙsûD¯\y¿ç™$(Ô4 ¿èyÚçÜs¿¤L߁°CÕ¿ïlìýļ]AGNbcu1RXS J091407.9-015949?ïûr‹§'T?5åÌe/?B5Ðl9ž?5åÌe/?ïí^«î/?gÚè¢5¿?b¡Sِ9}?gÚè¢5¿?ïØ}ò–'Z?n¨l¢'±?sÁ"r?n¨l¢'±?ïõAÉà—?B
îÍcs"?U|l4ÎC?B
îÍcs"?ïëÞLðA?]åmÅ羈?d!³Þ±'2?]åmÅ羈?ï¬OvjÒ?—¤êa†xm?"ì:âeKš?—¤êa†xm?ï­=w°L?'D	g°Yú?"°¿åƒˆþ?'D	g°Yú?ï•P'ú^Å?K°ÓS?Š«õýø²¼?K°ÓSAGN4FGL J0914.4+0249¿Þ4¼šÐ{X@@h&Üã›EÀ:æ*|«LJÀ<X˜џš@¦A¡µòÁ@Ìî?äž?Á!95«³x¿°ŸíË{?ðn"ü¡¦®@Ӈ[Ôg ?íòãâ"¿é.î•tpë¿êt»(_šš¿âMaa™Î¿×&IaÉ¿áÏïH²AGNfsrqPKS 0912+029?ïþiߺÄ?ï­Èw,h?)b¿–à"?ï­Èw,h?ïôA-ÐPn?Z©Š Ò?W}¤YßÄõ?Z©Š Ò?ïð¹L×
?aMJ#Ð?Ï?^fˆß²å?aMJ#Ð?Ï?ïü1÷tŽ?&&åÌgí
?>w&Núü‡?&&åÌgí
?ïõç'8uŠ?Y7sú·Ð?T1±vW¼ª?Y7sú·Ð?ïАÿA>9?z»®úH?w·€]Q?z»®úH?ïåøúì?rÀ3í†k?jú^4"?rÀ3í†k?ïÜç'cO¹?d
>{­?qŒ>Åi'u?d
>{­AGN4FGL J0914.8+5846?ï¿RÆŒA@D§t¼j~úÀ;U^½ûx²À<ö›]¾÷ø@b#¨§?úåP׈èq?ÒÜù€4à?ÑÃa~ ?ÿҖÀ¡E`@':g?ï¢w÷ˆ¿Ø÷£ei}¿á"i·S¾Ä¿Úa'¼]hç¿ÞÁ[)œ\¿ïÿíöé	AGNbll3FGL J0915.0+5844SDSS J091451.54+584438.1?ïøÖD^˜?@ñ{nüÃ?L¦ïX,s3?@ñ{nüÃ?ïñ€H9Տ?Yœ¦VÒÝÑ?\ÿo½ÏBA?Yœ¦VÒÝÑ?ïÍa7°ùæ?vT¶É?yOd=€ŒØ?vT¶É?ïÙ&ö ?Rù~ظ?sl"XŠS?Rù~ظ?ï÷IHo?HÄí"_RÚ?Qmó·i©?HÄí"_RÚ?ïÅAŸÿܑ?y-J1m³|?}_/ôcŒ?y-J1m³|?À86J?†‰1}·¡þ?‰õb	Ž?†‰1}·¡þ?ïyCm	?z¨¦oÈgF?×'`…ÊÜ?z¨¦oÈgFAGN4FGL J0915.4-3027?î›é¾êG@)g¢xåÅÀ9ÿϾï"xÀ<49O¬æ}@
¾ýVW{@º–ic?¿Èûà3÷?ÄŸ€
s@Ûc[+J@ª¾MØü¿à–/¢!M¿ÌqÇXÅʿ㚾È'Kž¿á™!¶3-¿çY$Hµ¿ïýü_Œ'…AGNbcuPMN J0915-3030?ïø "¨T%?Hgl±üÇå?Mu`?Hgl±üÇå?ïÜ'–¤?|x£ÿàH?qì4æKé?|x£ÿàH?ïç7ۑ?^ìJÞ£ùj?hÈý^6?^ìJÞ£ùj?ïÞƒ|?ODo>°«h?póp;¥û?ODo>°«h?ïè×¼-Ü÷?`òhN³@Y?g(D[ØÓ?`òhN³@Y?ï2]*Ûÿ? åv‡ˆÚa?™¿ÔW4ä? åv‡ˆÚa?ï‰rx *Ë?ŠmÇõË?£añ1?ŠmÇõË?ï<ÏڞG?€WÈ3úõ$?˜|æÓ&?€WÈ3úõ$AGN4FGL J0915.9+2933¿ÓxõŠ0E@Ey…H©¼ýÀ8¥	pÂ
À;-M@$³@áòNço?üN™´?¥à¿Ôu?´FƒÇö#]@#¿µ'@	kèhߒw¿Û·‰lü¿×üè]÷×è¿ÚnYåN£Ò¿Ù‡'›x–ë¿âcÆ®¥šY¿á—ÙÛ©¢AGNbll3FGL J0915.8+2933Ton 0396?ïüÅü£â?3"â+ô"?9Ðí1ãr?3"â+ô"?ï؆YÔeP?t¡Œ[c?s¼Ó	nÀ?t¡Œ[c?ïä¦Ð¹ÁW?nW¦`£˜?kY/)aðÚ?nW¦`£˜?ï—ÍÒA'?j&+Á¯w?Š8̋o›€?j&+Á¯w?ïó[½¶?YŽ/7?YõHØ;3ë?YŽ/7?ï=ï£!¾Ó?¦µá»l,?˜B˜X‰«?¦µá»l,?ï½Íl82?‡߆fJ³?€Œ¥	xE?‡߆fJ³?íù%Fû*ó?•@ÎÒ5—g?°6ÕÆnÚk?•@ÎÒ5—gAGN4FGL J0916.7+3856¿rõqSÐÈ@FؤTÞÀ9ÇÑq6À<Z«m×sð@}Š6OGf@ ôQvY?¶<Œß].k?»éß,Já¦@#³é¦ø'@ş\§ê?ïøª*s¿áŠ2¾™-c¿åV«¾	e"¿çøä¸{Üð¿èÛނ׶5¿Þú@MxAGNfsrq3FGL J0916.3+38574C +38.28?ïý"(¼6Ò?'	Àúý÷?3f¸ê]?'	Àúý÷?ïöÎCxy?YDZ˜ƒ
?Rcx‰J_S?YDZ˜ƒ
?ïåwu?oIqZڛ?jˆrô¡ú}?oIqZڛ?ïõ¤¾!š?@~Çct?T¶ƒÿ»Kð?@~Çct?ïù"Ò›©û?DÙ0ÏÄOö?I¬µ¨oF?DÙ0ÏÄOö?ïÖd†¾ö?u9ÙìÎ&?tÍòšôXô?u9ÙìÎ&?ï¸|֕M…?'ðË'ÝÉÝ?àÊP]Êè?'ðË'ÝÉÝ?ïßBVwí?\Ú/çè?p^Ô´;H8?\Ú/çèAGN4FGL J0916.7+5238?¢Ýy¢–3@EƒÖ¶Zš€À;96À<éaB:73@ ©³"Q]ì?ûbU)þK?ÈvnfÔ?Àž«;ØsI?ùŠý¤/ö@›‰¿ÜÏN¿â±/bn4;?ï[$éÄT?¶œ µÍ¢¿ÝåœFó¿Ú/¼TS¿è®ÏÁsÓ6AGNbllRX J0916.8+5238?ïþ-cKºû?#8
:+êG?-)Ç?+ÁÃ?#8
:+êG?ïò%Ep?X$ÕZŽŽ?[Áµˆ]À#?X$ÕZŽŽ?ïî=וÂc?iT<åëÄ?aÂ(1äø?iT<åëÄ?ï×ë?îF^?V~(ۆ›?t
`
<©?V~(ۆ›?ï÷ÉÑÞ@?Hê›Þ'à'?PmÄFF"?Hê›Þ'à'?ïÇ('‰?yOḨU?|tk租?yOḨU?ïåõäYl"?v­º¦ð`?j
·‹Û?v­º¦ð`?ïR¾¾Â?v¢Î͉/q?Œ«PZžL«?v¢Î͉/qAGN4FGL J0917.1-2131?èoè+‰+ô@2ëÊÙ­…àÀ:¿ÒóW{À<WMÒ@ê{áLá…@ÊA¤åþ?Àoºx¿ºc%¿,P@?üuuGª¹}@@Ÿ¼}¿ï»…|¬#	?ëÈóĈZ­¿åfl{S]u¿æ¼QքܿÕsϛY–¿á‹½m´8AGNfsrqPKS 0915-213?ïþóY9¾N?¿,ºÃìÇ? ÊhŠñ?¿,ºÃìÇ?ïêD÷*?nÇ(Ýì3?eéºá^?nÇ(Ýì3?ï©Z76«–?‡­¹×¿©€?…©r.å~q?‡­¹×¿©€?ïûvÙÙ®:?2þ˜Îáh?B$˜~.&?2þ˜Îáh?ïýœæSÔ?4Ýڐ:J
?3pâEgQ?4Ýڐ:J
?ïuØỵ̈?¢^Ÿþ¥œc?'Dç-՚?¢^Ÿþ¥œc?ï/e=V£?—Á{aª|Ü?š_]|•¤?—Á{aª|Ü?ï¶AøóÇ8?}Ð:Çÿl?'oË¥8?}Ð:ÇÿlAGN4FGL J0917.3-0342¿ì»"n›Ë@=æ»frû À;.Ɗ"lYÀ<˜-שŸ¡@!ºÏ ;Ê1?ü»-Çüƒ?Æ˛ÊKh3¿•ò†Hõ?Ñ%'×µ^?ÿCûàa¿ïûjÚim'?îƒÓ"g*²¿×Êühñ¿â×ßð•ÿ±¿Î-›™¤{¿Ô￀ˆühAGNbll3FGL J0917.3-0344NVSS J091714-034315?ïþ~™ÿ?«¢äµß?(k"wš?«¢äµß?ïòç?À?`æ"Š?Z1Û¦ûž?`æ"Š?ïì»c²›¸?h©(sÎn?cDœy_GÒ?h©(sÎn?ïõš"ýcÕ?@ÒQ@ªõ³?TÊÖx«6?@ÒQ@ªõ³?ïýS;L˜p?1r–ëb?5f&Ǘ@?1r–ëb?ïÍ<WãÛv?z‹†og	X?yaÔàxï?z‹†og	X?ïáÐ×Z›?|OÜ`t?n/)cÔÒ?|OÜ`t?ïÎÿ86?oÃG	vBÊ?x€p"ø¤Î?oÃG	vBÊAGN4FGL J0918.9-0625?æ|'­l4\@<©ÏF#ÐÀÀ;(ZµX<À<§ƒ]2L@ÅÐon¢Ë@Êô¯ú?ÏâXûå?Ó'{ˆŒ?ûûCµBm@ó^'í/Ä?ïã¯1±Rô¿Òþ"Õ½6W¿âòžM]€å¿èú'7¥ˆ»¿ÜõÿRÛð¿ã¢"Ÿg8ôAGNbcuPMN J0918-0628?ïø"²:?FÈX'm?Oñ´eàH?FÈX'm?ïíØÁURö?c@;Ÿ2s¼?b'>»+)™?c@;Ÿ2s¼?ï³.z´¡?zêÖ濱Ã?ƒ4aL_Ø?zêÖ濱Ã?ïáÐ'}Ðï?PÏ Á×?n/ØŇhÔ?PÏ Á×?ïðÇ]¢ ?[Y^!ꧦ?^qD¾†p?[Y^!ꧦ?ïºYiö
U?Ä'z?i¥Šd"¦?Ä'z?ï*;hè?'ò&Ö	‹?š¸Ÿ"šM?'ò&Ö	‹?ï1Êw_Ô?‡Žk€;*¢?™Æ±ó=x?‡Žk€;*¢AGN4FGL J0919.3-2202?ïæpOt…@2ù€ä–íîÀ;rûbÓÀ<²'{J@!VhÏÍ2M?û‡"7Üæ?Ô"D¾Â?ÂÊ·H×	g?íds²C­@Á5±]†?ëޖxÓ¿ïynìFå˜?à»ÙÊâ¿å5ü;Oa¿Âák)¿é$ô^NAGNbcu3FGL J0919.5-22001RXS J091926.5-220052?ïþ3cæ?%ÑâNJ#P?,Îß^<5?%ÑâNJ#P?ïð9"AT?aLH°Vu1?_ŒÙ©ìXq?aLH°Vu1?ïèQ¡÷û¾?k]\ã?é?g®^bك?k]\ã?é?ï÷¶Uš™Ò?8ÄRwÛïô?P"TÈ«U?8ÄRwÛïô?ïû£®Š0_?<t•A¢Š?AqE‡øÒ?<t•A¢Š?ﳟõÜÄ?‡«à÷"¹ì?ƒ'÷£³?‡«à÷"¹ì?ïÝq¼ŸœØ?z7êl5Ùd?qG!ÊNœ?z7êl5Ùd?ïèIöJ¥?]Æ;
>?g¶
&î+?]Æ;
>AGN4FGL J0920.3-0443¿àº…Côª@=ñ|^ö/À;+×õûÀ<W$ü8Ë#@˜"vm@wŸ©~+?Ë\(	‰k¤?´€ÊjÇÊ?äIRÄÈòM@	 ]Ötì?ïòãízÂ>¿èHyìU(Q¿èjd!舿ê1HKÿ¿á½¼>	P¿ïùœÙ¿úVAGNbcuTXS 0917-044?ïÿ_óŸcL?
ê¡zâ¿ë?'d¿ç?
ê¡zâ¿ë?ïõÚ
*®Þ?TÇhµz8"?TKë`j´¹?TÇhµz8"?ïò"­
S…?L<¸ó=Pn?ZئCNõä?L<¸ó=Pn?ïûæÕ®ë?%Ö<µAº?@d¨Î®À?%Ö<µAº?ïÿ¶QIÒ?ìД?\-:?"?ìД?ïÒZ%˜ôa?y4;@$ã?vÒí&wK±?y4;@$ã?ïìS´COF?d"̵)´Ü?c¬Kþ©9Z?d"̵)´Ü?ïæJ}/^E?[‹^·Op?iµ'ìšÌ?[‹^·OpAGN4FGL J0920.9+4441?ï*Åë 
Ö@Fgb(EÀ7ÉÑæèÀ;8àò¿@Ì8¢2ðB@#szK¹? Í&Ü/7È?Ár3y)6°@&…ô¡'-@®uµŽÂ¦¿œæAE£*ð¿Þ%[Z™ª¿å&=·³à¿æ°üÂ]޿ꨢ ÿ>¿íêi*fAGNfsrq3FGL J0920.9+4442S4 0917+44?ïÕzž,?tRêÁ?u|Âéâæ?tRêÁ?ï¿Õsm±?‹HAüécö?€
£(ÚÛÖ?‹HAüécö?î_¿‰ ]? §'"ñ"½?ªm#ó9? §'"ñ"½?ïß~ŽÈ¨?wٻӗJ—?pu@˜OX_?wٻӗJ—?îêMØU…?™\Ò¦Æ÷Í?¡["'ºC®?™\Ò¦Æ÷Í?îGzþMù2?¾LµE2?«ˆP°Ðâ?¾LµE2?í£dØI?¦j¦gã]?²äÙA¦ó²?¦j¦gã]?îjA–¦©?¤2v3ˆÐ?©[æ Q|q?¤2v3ˆÐAGN4FGL J0920.9-2256?à(:­ê£;@2¥…7âÅ]À:ÙjÿR[À<€[wõÚã@!$ï$©Á?öâñLO?Ն¥ 5"?Ö¬ƒP?ÿýf¤S1?÷°o̖œ¿æx="ßEu¿àNÏÜKÅÑ¿ÎK*
j'¿»Õ9'ØŒô¿àš¥½ê0á¿àõ–AGNbll3FGL J0921.0-2258NVSS J092057-225721?ïø¡¯ñ'~?BÀµð™c?My@†&UÍ?BÀµð™c?ïÀΝ"?',Õ`n#¥?˜±…};Ã?',Õ`n#¥?Lqó?ƒŠA¹;&?ˆlêbT¡?ƒŠA¹;&?ï—â®F¶?l$ bÔh$?ŠTx¡S,?l$ bÔh$?ïõÌñhk,?OÏRì_Õ?Tfø/èU?OÏRì_Õ?tÊá?´¹ìñ~‰¨?¥÷¾§jõ?´¹ìñ~‰¨?ïÝ\Ö´q?ˆ÷áãR½?ˆˆ¨ÆãGÆ?ˆ÷áãR½?î(AcçIê?—kN^†ì?­{éÄU?—kN^†ìAGN4FGL J0921.6+6216?Ƽt^´k@Dᆘ5À8LPíX^À;ê"lXî¯@"ýð[GN@ÇìoíÏ?œMÜ#N[$?µFß•d¬@2è8ªk@¾j£Œâ|¿ÆÉ™;¥È¿áΪó^1¿ãÝ_~Ù¿å‹V	÷Ї¿èém¢ð¿ì,ÉVö†ÚAGNfsrq3FGL J0921.8+6215OK 630?ïøAøp?M)ÞÌWÊ«?Nø¨¾,ý?M)ÞÌWÊ«?ïòëÐ9L?dK¯CY?Z(_>ܹ?dK¯CY?ïßt^™
?u¶èç¹ýÝ?pxEÈtk?u¶èç¹ýÝ?ïÿ…T#÷?ìÒ¯4n?œ%@ðœ?ìÒ¯4n?ïõ¼ÍXì?Q§¾'ç$?UʆuÌG-?Q§¾'ç$?ïÑB³Œg‹?}p8ËÆ6	?w^¦Ezæ­?}p8ËÆ6	?ïÒ¢Pï©?€}V³¼¿?v®×pÎ?€}V³¼¿?ïþû5jðå?䞆Fþ ? L¨;)Q?䞆Fþ AGN4FGL J0921.7+2336¿ææŸçÖ,@ElÍJ¡À:<—FÙeÀ<xÀŽÐè»@¶õ¼/E¾@y@þÍÐÙ?»Ø5õ…S?`¢1Áä©r@K®+÷Տ¿ã­ÕÀ­¿æÝݖH¬A¿àîŸéiæ¿Ú$;ɄĿéÔÞF-⿸«äIìPAGNbll2FGL J0921.9+2335NVSS J092145+233548?ïü…z[nn?3¥³¥½Z£?;Ô+çãÂi?3¥³¥½Z£?ïö](ò^ú?TP¡?SE®ey›"?TP¡?ïía­Dc?bÿ·c¹¢Ë?bžRº"Å%?bÿ·c¹¢Ë?ïûs{x?0ϲ‡Ö!?B3±š'q?0ϲ‡Ö!?ïøͳ@x…?CÖ;MpK?LÉ2n¡pc?CÖ;MpK?ïӏ¹ñÓÂ?yаË$,5?v8"÷÷Öå?yаË$,5?ïã˜Oäç?yrȪÂ?lg°K3pu?yrȪÂ?ïõ'‰Ü¸'?FºU3c´?U°ìʀ°¬?FºU3c´AGN4FGL J0922.4-0528?Þ%iÏ°
@=푼U†DÀ9õ×CHT-À<WBXj$a@í™IÁÉ@[A9†3‹?º½ó×þ"?Áû¿i!@¿l\I¬ò@I1!`"?ïú=³¿µ?±'Ò*.Ò¦¿á7€—9î¿äW~Áüå¿Þ:Ó²¿êc'@ßÄ AGNfsrq3FGL J0922.4-0529TXS 0919-052?ïõrzhH`?_Ýôñ8ÑÖ?U2¯¹?_Ýôñ8ÑÖ?ïÜ
AøGû?kŸ«IøÙ?qúÞï>Z¼?kŸ«IøÙ?ïԓ¼é'?xØZDôÄ?u¶}:HgV?xØZDôÄ?ïrˆ¢j<y?q:åÀ
?'®ë·ßÚå?q:åÀ
?ïªýÞMäÌ?'M,ãsŒ?…@ˆl†Í?'M,ãsŒ?ïo
uÎ'/?"ϳk2?'QDƒL,?"ϳk2?îëœi¾Æ¶?™xw#[÷?¡F9eËbŸ?™xw#[÷?íGp•Ðr…?›&Thè?µÄ{Qê_X?›&ThèAGN4FGL J0922.6+4454?ëDG¤üœ@F‹«ud0+À9»ˆpSOÀ;;èné§@lY­ñ?s@µyyh¡ª?µºÎaf;7¿·B~"%¥@¨š¾\ǁ@zxnљæ¿âEà_PÈ¿ëÕ®Þ]¿æ4ò»sÞõ¿ã'
?ىʿïò5ýgõ2?îÈïÈzWµAGNbcuNVSS J092235+445749?ïü>;ÇMÔ?8˂ó®n®?>#Š'¹?8˂ó®n®?ïõ}¡7ë?SH{{ï¸&?TÅ4ÊÔ?SH{{ï¸&?ï¨ãÄ	?"b²öa™—?…Ç>¬é×?"b²öa™—?ï÷MmQ?C!:σ€?Qe–û¶?C!:σ€?ï÷':L#'?Vÿa©yÌ?PۋîiŒW?Vÿa©yÌ?d¿å*3?‡Y'/¬"È?€žÐ‡7?‡Y'/¬"È?ï/‹õÛӕ?"¼PRÓ·x?šM"_?"¼PRÓ·x?ïM#ua<A?üA¹Æ¦;?–['UE×?üA¹Æ¦;AGN4FGL J0922.6+0434?±~_Må³@A»´_½ŒÀ9Òþ?5 À<7•óëï@šÙlmf‹@͉ößÆ?°&Ëƽi-? 	ߧÅ×:?ëG©Â†¢Ç@=zœ©C†¿ 'Ѐ>T¿ßz}	@¢¿ç.,Ε#é¿èëaŠR¿ç»š?±Æ·¿ÖŽƒ»áÂþAGNbcu2FGL J0922.7+0435GB6 J0922+0433?ïÿ•;!?d)Â?mRTLvJ?d)Â?ïö¾‹K?Uœ¢Fi+u?R'êX¶hõ?Uœ¢Fi+u?ïïfa«8?aç Y="F?`™ž/9b?aç Y="F?ïÿ'2©å>ÿHٔ3ºø? 8 ·¨>ÿHٔ3ºø?ïÿC{?Zs"-ßz?ûßÒÊ?Zs"-ßz?ï×AGùP?vg¤êޘ@?t_\.C¨(?vg¤êޘ@?ïÛ
†"ˆ?yråFá{ß?rys¡qÜ?yråFá{ß?ïÿ,ñÙ)Z?L»R?ƒ/?aÀ}º("?L»R?ƒ/AGN4FGL J0922.7-3959?¾>˜×|Ô@ƋýϤÀ9sÒì¡~jÀ;ݸçì
@}"£˜öÜ@ƒˆ›D"…?¶hÛ¡%ÿï?¾¿Ïä.hH@Aƒùdo@Eìs±(¿Øæ4"E¿æWãa
áë¿éZ~›çQ³¿ã'ÞÑ·¿ì
ÓØZ¿ïÿƒmÞ)ìAGNfsrq3FGL J0922.8-3959PKS 0920-39?ïûHÛ2"?<ÿa'kÕî?BܔL\?<ÿa'kÕî?ïæЂu û?vÍ^©7?i/}™ýMc?vÍ^©7?ï×$ÄÛfÄ?oÔò€{"‡?tm°‰.?oÔò€{"‡?ïÿûÆo?
"…5¿ñM?—)´?
"…5¿ñM?ïîJƒåZì?db~Qv	?aµ|ˆh?db~Qv	?栗I~
?¥˜ÎÅ)Ó)?œË¯ñÙ?¥˜ÎÅ)Ó)?ï_vŸ»éó?'kpÿx?",Êó¤?'kpÿx?ïü¾ Ùá«?.òHâρ?:úuMÉ/?.òHâρAGN4FGL J0923.5+3852¿ÃvŸ»éòð@F½inX£/À9ÛýåsŒÀÀ<"æu@V¢NÉç•@ß09ƒ¯M?¹¡®æÝÅ?ˁR:Šj}@
¸e6»~@ÕÅCìi¿ÙÑãl'¤¿åZ:8
3¿è›!>>)0¿ê'?_†¶¿ïÿöût€¿Ênà]xV(AGNbcu3FGL J0923.1+3853B2 0920+39?ïÞ$SŽY?o{ß/"?píð¼ËÍ?o{ß/"?ïô5X@L»?VO˜¾°-õ?W•O'¤YÔ?VO˜¾°-õ?ïA9†¼û§?òKà@?—ØÏ-‡õ?òKà@?ïò"(¯Í?Cç|øX¡ç?ZÙÅÊFÂ?Cç|øX¡ç?ïÝBðY]®?mâ̸/ÔÕ?q^‡îÎÊ?mâ̸/ÔÕ?ïÆÚN·ëa?€ñÀÖV.Ò?|'Ø…Í¿Ó?€ñÀÖV.Ò?î2ªà'¦?žŒOóu?¬ÞuRÓ¼Ÿ?žŒOóu?ïdm,ö?y†á‡Ï)º?Œ&ûï–S?y†á‡Ï)ºAGN4FGL J0923.5+4125¿Õ×ã%\d@F¼	ԕ+À9"+¸ënÀ<i3—Ý÷@QÞc£"@xAàu >?®<ÃÇ
–?²ºýíV/7@÷×ûÕ@
òÍtg†¿ËæJâ§T˜¿ÝOÍ¿å×6èÊYU¿äe8Ó¥"¿æÿe I¿ìÃßâSGAGNfsrq3FGL J0923.3+4127B3 0920+416?ïþkT[™?Ëa"Žb?)F/c~¥?Ëa"Žb?ïõr—ïl×?V>²*Ä?UÏï«ñÎ?V>²*Ä?ïò"'ûغ?OàòÆ
q%?Z×°'¾êó?OàòÆ
q%?ïޙ	j¦¬?YÜBý
?p³{E-J(?YÜBý
?ïü€áÕâ?0îÉ	
ç?;ÿØO5Â?0îÉ	
ç?ïÔ¦(8j?xA'úŸ•?u¬úL÷Oc?xA'úŸ•?ïå·aM[?p̞@×½j?jHžwÍ]–?p̞@×½j?ï×R"(¼?{øœr½Ä?Š+l´A?{øœr½ÄAGN4FGL J0924.0+2816¿âÈFL.p›@F7ë¯#dÀ9î—ÁREGÀ<zãv\}¯@]ðáy@.þOü—–?¯‰N?J¿¦&ú?̞ª?ñlj	ÿ]@A<%J<d?îŽÃ|Áò¿äÒ8\gà¿èÐ"uE&¿à×J4¸¿ç>àæ_E
¿ä+"XÖ[AGNfsrq3FGL J0924.0+2816B2 0920+28?ïÿî­$ï?:ü¶¾Çú?b$àh:?:ü¶¾Çú?ïöô«¹è?Q´×d_¸é?R¨ˆ~Ïù?Q´×d_¸é?ïö–ùðá?C7©²(f?RÒLøÑ?C7©²(f?ïþéš›?4Ó_õÍ?!o<çz—³?4Ó_õÍ?ïÿz<˜?öŸÉŠ{?¼(ª}‰?öŸÉŠ{?ï×oô7R…?u I'ç|³?tHÎY=?u I'ç|³?ïò÷—·ÓR?`f#JßÚ?ZÐrÌÅ?`f#JßÚ?ïýZtÿ?&·¾¹›t¦?5/πt¤?&·¾¹›t¦AGN4FGL J0924.0+0534?éaÍ.5aP@B#Bþ'Q~À:ô'ÛçÀ<ˆë"²'@ ,üÉÚ¨@â…Ãù¿t?©Ú—O¿¨é#šŽâ?ç·4Ã@	!'Ë?ïœd…D¿é᦮U¿ä³ñTk'¿àÏ;<1¿Ñ[=E@¿áãXàÿÇAGNbll3FGL J0924.2+0534RBS 0771?ïüõt
é¾?+ªsUôÆF?8T`N¸É?+ªsUôÆF?ïóú³öù?YÞärÌù]?YÎ
f—­ì?YÞärÌù]?ïöFõ¡œ?BÕ»Y[¬?Srx¹º?BÕ»Y[¬?ï÷"³Î¢?4—î¸^ì?P֗ûVœs?4—î¸^ì?ïû+% ?6ʏŠÉ`?CS"*º]¥?6ʏŠÉ`?ï͞Ê8¦m?z3C®;vS?y0šè|=W?z3C®;vS?ïùŚÃ)$?RÉK Î}?Hé•`Â3I?RÉK Î}?ïȲ~ö]È?l«†h¨Í¢?{¦À¦}Gž?l«†h¨Í¢AGN4FGL J0925.7+5959¿äKÃè%ã@E sÞ-èÀ;-Ówá¹À<àì^b‹æ@ ¤|Ö?þb7G"ê?Å1®ù¨"?¨ËPö½Œ?ä8j¤ @"Zî?ïòÆ@Á'/¿Ö–"'I¿¿á´b\Ô¿á[þ˜÷³*¿ÔOd!ȿۏ²tƒàAGNbll3FGL J0925.6+5959NVSS J092542+595812?ïþ {Ø_õ?+×Ìi_?%øDæ ²?+×Ìi_?ïö«ûÆàO?RjChQ!'?R¨˜»a?RjChQ!'?ïö¾-!Ì.?U—{jµ?Rƒ¥î…)?U—{jµ?ï÷+c°ÿ?3]TKò±o?Pý¨Å+!Ó?3]TKò±o?ïþߦ2?#Ѭ,.·B?/2#aw%?#Ѭ,.·B?ïØ­1À±$?tî*õT$?s©g¸qØ?tî*õT$?ïôÉ£w"à?dµ›%µo,?Vl¹WŸj?dµ›%µo,?ïæøÍØ?V¬^æU§?i÷=øè@?V¬^æU§AGN4FGL J0925.7+3126?ï/{BÁq@F­"àÀ:…¥>éIÛÀ<«ªïê@VÿYfú@ƒ¸¡œZ?½‹.`ªS•?™€È½H X?ÚæÞP­Â@'4ð!»'¿ÒJÎZk†a¿àÜ.1k³¿ä±3¼Åï¿ØÞd$í ¿çáӟyØ^¿äWŸ#FVAGNbll3FGL J0925.7+3129B2 0922+31B?ïüðm³.8?)þ}ÀI?8|"Ìÿæ?)þ}ÀI?ïöÖíÑÃñ?Qœã'ž8æ?RR$Â,ŒÝ?Qœã'ž8æ?ï÷ütôã[?BF_>|?P
!<?BF_>|?ïô>ÜÔæ??äf# ?W'GîV4j??äf# ?ïù9}á=ƒ?C€ ž2"?Kš_ü?C€ ž2"?ïØ¦#A?xVOlY?sù¬æ껎?xVOlY?ïñù[î_¼?j²Òِü?\
HTºçÒ?j²Òِü?ï×ÖÔôŸ¶?`¾
%–'&?t•¤œ î?`¾
%–'&AGN4FGL J0926.4+5412?àæ>w
@F	š¿3‡À;wžYóÀ<؂ ×@ 6PiNù?ýÙ¤K¤CA?øh;ӕ¿?²ÛóÚ­¶?ðÁàŨ]@㉠þé?åë¡òYN?×_×Ár{ž¿Û·¤F›ÅÄ¿ÞqIþ7(¿ã ®Ì0ś¿ÕDzãíAGNbll3FGL J0926.3+5409NVSS J092638+541126?ïÿ…æ*ä?€œú´°?G;b(Ð?€œú´°?ïõ²?
Š{?T5뼪?T›'eiy?T5뼪?ï÷ëͱ?<"ʳ°?P)øuq¡Ù?<"ʳ°?ïî;6âÀ)?A9¥TÍé]?aÄÉP"?A9¥TÍé]?ïþ52šd£?#pòpÊ<U?,¬Út×ß1?#pòpÊ<U?ï×c´Ze&?t¹¬ùŽœô?tN%Þ|Ë?t¹¬ùŽœô?ïö­^¦B?fQÒêúÞ?R¥B¾ò;Ã?fQÒêúÞ?ïËÀkћz?c1µyZõ?zÊ3ƒ%?c1µyZõAGN4FGL J0927.2+2454¿ëøëâøÄ^@F2wpyåŸÀ;0èÈ«ÕÜÀ<½{µƒ@*Wú½ËÓ@ ߛÜiù?ÑÁ‰7Kƨ?Æ#G'Ëvá?ó6¯Ž)ú?ù†ßúüá¿ïØgHðŠ?ïÿ¯"AôA¿åŽvàÜú¿ÐèkÄt8·¿ïûÆ«±Ê¿ãì5YAGNbcuMG2 J092720+2456?ïóŽŠ¿.?S/ÁJ¢å?YàãG÷@?S/ÁJ¢å?Âӄ?Œù3H†öb?‡Zω‰ŽÜ?Œù3H†öb?ïUÿ¤ÌŽË?Œ\¦"ÁÒû?•@k•¦?Œ\¦"ÁÒû?ï5fi@‹`?|Ò¯"ya??™S2Û^/í?|Ò¯"ya??ïæöüm›±?g}O?
?i	Áþ|?g}O?
?íûH#–nR?¹¤aÒ"ø?°%¾ãLo?¹¤aÒ"ø?ïôË«î?"ao'§:?œf"z>?"ao'§:?ë.Q»Î<?²?bS	Ñá?ÃïF¹Ç?²?bS	ÑáAGN4FGL J0928.1-2035?í»¡ÅsMf@5x¦—®ÞÀ9þç×NlÀ<c$—Žý^@ÐOo õ@Šúšeq?¸pÀ\Àº?¿å©érö@Ò}{Uá´@ºÉ,YOR?ïªFà!q¿æöÏՕɿçAȌÌ+½¿ç€Ú")=¿êï$°¹pÏ¿Ò/)"ä¤AGNfsrq3FGL J0927.9-2037PKS 0925-203?ïý}µž™?'kåˆ?4Q|Íz?'kåˆ?ïòfØ÷?`áŽ\Ë?[Ç3NÄ°µ?`áŽ\Ë?ïäÛKb ~?o¼˜Å?k$´¹\aé?o¼˜Å?ïýâb¤ÿ˜?ÑèèíX?0ìëo¾ËR?ÑèèíX?ïùä¸PéÒ?Bt}b!Ï[?Hmûî—[?Bt}b!Ï[?ïÎ =@ö?Zç	=†=?xïö[à%B?Zç	=†=?ïÎGv6=)?y)çŸÖÞj?xÜD̈́¶?y)çŸÖÞj?ïùgý‡?;"*}ÂÝ?Jc§ÚÈe?;"*}ÂÝAGN4FGL J0928.2-3048¿ÕH΀V&¨@,éáŸÂ¨‡À:Rۗjë0À<(<˜6Ã@,LÖGtß@ùúÊ9?ÁÉõA‹¾?¹Q"º•?ö]‡ëlm@¿!"µ?à7Åü-ã¿å—Ae%Ç¿æü¥Øl=¿é6sXg¿ßc¼ÑG¿ïø*ÿ2$ÀAGNbcuPKS 0926-306?ïþB‹?šíl¿'y?+×ï'<š?šíl¿'y?ïë>•š?jE£™ë؏?dÁj¡ê
?jE£™ë؏?ïípÜ6!O?qGgë/?b#ùù8?qGgë/?ïö÷'Àƒá?5Cßš©Û?RÚf;ô?5Cßš©Û?ïýïø~‰ü?&šÛhéôá?0€:W.ŒÐ?&šÛhéôá?ïoœ't?˜pk«}Oj?¤ò–ë&?˜pk«}Oj?ïß-ç¼3Å?{ª'äØ?pi&µ'"?{ª'äØ?ïÂügLÈä?k¼ˆ/»ç?~ÌSlAÿ?k¼ˆ/»çAGN4FGL J0928.4-0415?ÖzFÀ%A@?Ü_õHíÀ:"a‹5RÈÀ<oÙzZ91@vœ#·•-@Õ;f›Ö?Æ˃ ±P?º8öLÖó?ñÐD¡À›@	¥ŽÎºb½?ï¦pý™s¿ä2î4%¡z¿çe`!Ràø¿æc¤FÞâ¿ïÿø]ˆò?ê/†€b;	AGNbcuPKS B0926-039?ïއMkê?­ ž$% º?p¼YÖ®£?­ ž$% º?ïôÿˆ‰Z?TÄÎ7CUÆ?Vüµ3Ý4?TÄÎ7CUÆ?ïã¾TÓ°°?q)´T<	Ÿ?lA«%pŽ?q)´T<	Ÿ?ï÷ôØ|¬?8×$¿H<>?POD¨s?8×$¿H<>?ïþ8ýÍu¿?2bTp
ñš?,p Ÿíі?2bTp
ñš?ïÍã;ŠUë?~‡`Ç3?yb16"Ž?~‡`Ç3?ïè󸸲}?wÿy'uC?gGVkʑ?wÿy'uC?ïÓ_@µÛL?e¾æU"?vP_ü?e¾æU"AGN4FGL J0928.5+4048?Þ7ŸdÅã‹@G7žYò»À:ÝҜ¦šÀ<Âc:aûž@²Pt·?ÿÆ.¢<Ö?ÇYü ¤ü?¹1ÀíE"2?òB¸ý/¹@ z~¡Eµ¿àå´àFý¿æžã…uö¿ãk®Œp¿Øåøƒã¥¿ářœô—í¿ïÿö$´ë/AGNbll3FGL J0928.5+40481RXS J092837.8+404858?ïý[¥ Â?-ffî
`?7u#Z7_Ä?-ffî
`?ïõ‰^ãæ?W~Ù²2÷Š?TíB¦'Mu?W~Ù²2÷Š?ïó²stÎ?U|âžW-ã?X›™"Ãð?U|âžW-ã?ïîJf^6u?CàÓ³æy?aµ™ªL?CàÓ³æy?ïü˜ÉSàA?5í°ñœ´?;9³ÅÆV?5í°ñœ´?ïÕ	Ÿ»ó?vv¯f¹ã0?u~{1Þ¹?vv¯f¹ã0?ïömú'?`iÁ'lŒ?SÅ$K1¬H?`iÁ'lŒ?ï¯c 8o2?p\DkE?"'ú#Ce?p\DkEAGN4FGL J0928.7-3529?ãÍúR¹X@&p4 ½À:B ½å©=À<0d~.Ú@<gm!–~@ã`ݐio?»»žÕ(ø¿cD§"œi?¤£áÈÂ@ҐöÝÂh?ьPû"¿èKƒŒÚ¿â`c&¿à3Vn¡žK¿ç/Ë¿Üyh¿Ú/\#—^×AGNbll3FGL J0928.9-3530NVSS J092849-352947?ï÷
:{&?B'"ÕÌ
'?QåŠÂ;þL?B'"ÕÌ
'?ïèa§©–?tæOzE§8?gžX—'?tæOzE§8?ïêj†Jv5?eµívá>ç?e•y'Íۈ?eµívá>ç?ïëFäôi?J""þ)ò?dü¹=g®T?J""þ)ò?ïÔv×ͱÏ?qA¶Ns:?uĔ¨øŠ?qA¶Ns:?ï|Ž
ŸOç?˜ÍÑ9?n>Fî™)?˜ÍÑ9?ïÃë8Œ}@?ƒá£Ñp?~
cžD€?ƒá£Ñp?ï¥6©Æs¨?rª	nâ¸?†²U‡ƒÝê?rª	nâ¸AGN4FGL J0929.3+5014¿Ú‹þOj0@F¶™÷LÀ9Û~@w¿À<%êÅÜÃ@/Y­€@Ê%Ðt!?¥C'«¹µ?¢ó~½JM×?ûæ8^_
@ò{PÞë¿×R]šåÊ¿Ù^ØO·Î¿ãž"jc ¿á»ßá§z¿ßfÚ?&0–¿ënxÿQæAGNbll3FGL J0929.4+5013GB6 J0929+5013?ïþ\º‰?ûû'† ?*>´°äŽÏ?ûû'† ?ïø*™¸?N#Gÿº?OU¼¹ì-?N#Gÿº?ïô1—@'±?cM;3<Ú?WœÐø)î£?cM;3<Ú?ïûæ%–ðû?-:'O»˜g?@ghäëm,?-:'O»˜g?ïýÏZŠ~ã?"c¹=K?1…-–j¼{?"c¹=K?ïÖç"Áÿr?{­Ãü¨_k?tŒn£Ï?{­Ãü¨_k?ïókù^Œd?i$œÖ¿?Y(
­)0?i$œÖ¿?ï÷¨‰‡¹Ù?C8~Š€×?P®íH'L¹?C8~Š€×AGN4FGL J0929.3-2414¿î¦ÒîØn@3/ÃøôõÀ:úù€‰þÀ<›>»&²@~¥¢fr?ýTq÷" ´?Ô¿""Æ?Ùè'¯qr@  F\ä@b35e"?ï¬LŸ?ö»¿âåAã¥+¿Ôy;U@¤¿ã¸ÀÅ­¿åöü¿ïþöë"GùAGNbcuNVSS J092928-241632?ïòôcê‹$?Qû4÷ÕûO?Z8	íxÄ?Qû4÷ÕûO?ïÄRˇ…ù?}‡@‰¥Ø?}֚AwK?}‡@‰¥Ø?ïfñëY?S~&&}i?‹æCŒñÈ?S~&&}i?ïzg$Qn?j=^¤âã9?³wŠ
%?j=^¤âã9?ïß¿N›)Î?lNSÂM?p X™­éB?lNSÂM?îÚµ'R?°ÓŸŠ˜vŽ?¢_Ô²Ý?°ÓŸŠ˜vŽ?î§z¼Dûn?š_¤4»-?¥ˆT9"&?š_¤4»-?íʄ&Úy"?•»îôtD?±«ÞÇâ\u?•»îôtDAGN4FGL J0929.6+4621¿îB0×cS·@G
 r~À;"Îa!ƒÀ<"«ùiä@þžl<>J@|ïÅYb?Õìé¢Æi?¿·ÿãz?ߘ¶…7·Ò?øSƒ""_?ï£XK±¿èo~¹Å¿ã?æŸÜ©º¿ëBµþ,Á¿ã.¨TGñ¿ïùm¿¡9AGNbcuSDSS J092922.75+462046.4?ïýñwtg?.˜"»}?0wÔjØhp?.˜"»}?ïÕ'f÷/ø?}ˆ¸(@2?ulL•–?}ˆ¸(@2?ïµY'lI?€–]Ã3TÄ?'©ŸZR£½?€–]Ã3TÄ?ï–ã#Œˆ?pL™åÈ0?Š|Ç0=¥÷?pL™åÈ0?ïø¼If²?M	°X?MÛ·"?M	°X?ï6µÅI?¥S-<Êº?Ÿy-éGV×?¥S-<Êº?ïFy\¾?˜Ax.6‹?œ×0ÙÌ??˜Ax.6‹?ìã7PüÞ?¤Ê‰
SŒ?¸æE€f'?¤Ê‰
SŒAGN4FGL J0930.3+8612?éùó¦LÒ¹@="%¿­)™À9h›WûQÀ<Eyõc¶@MßÇPa@–£E?¶J¸ o÷Š?¸y/ýÚÇó@u5'Ì÷@ˆ¿6Œ.!?·ö*NçD¿ß·RDËâ¿ã7³`<οá²+–†¿¢¿é?qdÇ)ö¿ãcBZ£‹AGNbll3FGL J0930.2+8612S5 0916+864?ïý¼N${4?!ýãÒ_?2ëêY.?!ýãÒ_?ïõ݂&¶M?UžÞæÌp?TDûúE@?UžÞæÌp?ïé>š;øK?jòùÇØ¢h?fÁe°Éäù?jòùÇØ¢h?ïõ+ï®4l?Aäo™ýÄ?U¨ 'šç/?Aäo™ýÄ?ïúEã'ñÐ?:Ô^e.¨?Fès›˜d»?:Ô^e.¨?ïÒniaß?zZ"ê	œ?vÈË8Š¤v?zZ"ê	œ?ï¦0õÚüÕ?‡äwW]0ž?†sÂ{'ZÍ?‡äwW]0ž?ï䥣'·?[éÑê=?kZå[p"?[éÑê=AGN4FGL J0930.5+4951?¦ËÄG/N@FØwîN&ÕÀ:ÌÉÀ¨ÒÀ<È±µR@!t1¹áb±?ýP2é?Áǧ‰qX]?ƒMŽF@?Åö€û=" @÷ŒV:_¿àÕ¿ðEwÙ¿ä<ôb=ú¿ãooŸ?‹¿ß2ù<†ª¿Ýnm[x Î?«Á^¥…iAGNbll3FGL J0930.0+49511ES 0927+500?ïÿDI8¶³?	Ÿ'U¨Ì?vßiÒ°ñ?	Ÿ'U¨Ì?ïöÕÖ¥'u?Sêíý˜u?RTS8ì¢?Sêíý˜u?ïúׂeþë?2'•]ƅS?D¡÷(û/–?2'•]ƅS?ïü`È0ŸŸ?'"^ï5—»?<ùÀvüyš?'"^ï5—»?ïþ³'ßÿì?^p§ËŸ?$ÇÒ¿QëÈ?^p§ËŸ?ïÛ["F\l?ræӝÇ2?rR=½åN/?ræӝÇ2?ïü§Sý"Q?KÖ*¸§æë?:Å_Xr¸O?KÖ*¸§æë?ïójÎU
#?MjӇßi?Y*c]šL?MjӇßiAGN4FGL J0930.5+5132¿ç¼j-_""@FªJ¾j3{À;¿°ä8úÀ=u=™¾ƒ@ D߀®'"?ü¶¦4²4?ҒߪJ?Ïv³»ƒÏ-?ûtÓçsA@@¶©
оt¿ßÓ^Kå± ¿ïÿ\‹/ô?ïüSme^)¿ã;§««¿áÓÌ/îÛ¿ïÿþó…õAGNbll3FGL J0930.7+5133NVSS J093033+513216?ïûÒE??bI(?Cì¸Û°±"??bI(?ïô|YwÁ?Xv	CŽÐ?WÉ.Óï(?Xv	CŽÐ?ïÇø¦‰0?zyýA;¹?|¬ÂG6?zyýA;¹?ïÞÒNÓ?W0xà:ä•?p–؆­ÆZ?W0xà:ä•?ïúqP­Ë?IO¹; ?F:½Õ­ü?IO¹; ?ïÖ¼7(`F?sÓue	S?t¡äaÛ?sÓue	S?ï¡ØdÛvß?†&™þ¶'G?‡‰æЀK?†&™þ¶'G?ïªL|°TÇ?w!kXhIß?…là×Zj;?w!kXhIßAGN4FGL J0930.7+3502?ßåë¤Ò@G`ÉÀ¨ÒÀ;0f('ðÀ<ܾ•Òd¼@ÜY·Vmö@+À nŸñ?É?æPl?­HPÑ©«`?ã"cßùOb@î¿æµ?ïê"Q€ü?·ÌZ ²Òü¿æòƒàÊ°"¿Ð]ãŸ''¿éÔ+{¯¿ïøÿ?æŸÝAGNbllB2 0927+35?ï÷j[Ø1Ê?Eyþ|s?Q+Hx×¼œ?Eyþ|s?ïî1ýº;·?aåðe^?aÎw>¨ð?aåðe^?ïБ]5V?n¯€ƒm?w·Qo<Ã?n¯€ƒm?ﺲßÌêæ?by\ÛHˬ?SH#Þq?by\ÛHˬ?ïîQÊM²?\YJÆæ…?a®5ïcm=?\YJÆæ…?ïºÔù?ŒÈ©Ä¸jæ?yy"<ÑÎ?ŒÈ©Ä¸jæ?ï¯Îê‰KC?ƒŽöQzKï?"EZíQ?ƒŽöQzKï?îä#|˜e?‹Dûœ=ïÂ?¡½È3F9±?‹Dûœ=ïÂAGN4FGL J0930.9-1015?¢DáLyî@<µ?á—_-À:Z'¹hÀ<vö=Ÿ@æF×)òî@WUÿæՍ?¿]ç;ãÛÝ?´zr!…‹Æ?ñ+!Z³@ê$O?®?ïÿÕ%t.¿ÝÜxüÁE¿äŸNyà–®¿édŸ;ïð¿ááHtEL¿ïÛþ~ÀAGNbcuTXS 0928-099?ïþ.&.?Um™XO¦?-˜Þ[&?Um™XO¦?ïöIӈ¨±?U+Aû4­ž?SlYW"¾S?U+Aû4­ž?ïïžÞ§ì?[€2dá?`ïaað¼?[€2dá?ïýo4žË»?µÀªIQ?4†\Aå!?µÀªIQ?ïþêË?W_Š¼Ã¡?!^¯Z^Þ?W_Š¼Ã¡?ï׳{uŸÈ?x'üÙè8Ã?t&BD€0?x'üÙè8Ã?ïâw˜à-Ÿ?q#¥ñG?mˆgOìè¦?q#¥ñG?ïøaà±??%
­œ¸þ?N{¹ƒŽ·??%
­œ¸þAGN4FGL J0930.9+0033?çn~ù¸Æ¹@AŽ'bEoÀ9›õœÏ®ÿÀ<G^ñýÞ¾@L°·mj@Ƭ!\?µKÌ ñÁh?Áö*¿@ƐšíV°@ÿ÷ªÖ¿ÉjW·¡íP¿åþŸ­¯Ñ¿é­'©èò¿ë0߁w^¿ïÿØþ3w&¿ïØAªÅ;AGNfsrqPKS 0928+008?ï¼WW»äÙ?°+†1™n?€ê*M?°+†1™n?ïã¼y²7d?n¯gÅ䶰?lC†HI;þ?n¯gÅ䶰?ïÜláïb"?oÒ?¡*Z?qɎõæÀ?oÒ?¡*Z?ïŒÈò'qF?wàš··Hú?ŒÍÃ_J…?wàš··Hú?ïéÕÉː?eWÐè5—?f*6;N«L?eWÐè5—?ïŒ^‡—/ÿ?šœ`vÌàÐ?Œè^TÈ9?šœ`vÌàÐ?ï¢ÓÙÓ½Ï?†…a½Úø|?‡K	œ>˜?†…a½Úø|?ìãFÖÂß?¦õ¶^£â?¸ç
ǒ
?¦õ¶^£âAGN4FGL J0931.2-8533¿ç_Չù'QÀ8:dž;îÄÀ9ÏÝ;¯ÙwÀ<H~@WZ¶"áÒ@6Øôù;Á?´4T_AÉ?™òĒZz?ã[é4â`@Û3¡íûñ?ïðDÁPï¿áŽÉý³ø¿é•lä.é"¿âÒ5!Iü£¿ê';ÿŠ;¿ïÿÔ@ßn:AGNbcuPKS 0936-853?ïú|Vxîº?F±<²Ù
&?F¦-Oòû?F±<²Ù
&?ïöQ—ª*?WT'×ií‡?S\э¶íT?WT'×ií‡?ïÜÂHíã&?q‹"µ1Q¾?qžÛí¥3?q‹"µ1Q¾?ïþu¡l̲?íe"> ú?(¥æ8%>o?íe"> ú?ïùúVë°?Bj]R8?H¤–"?Bj]R8?ïو™¹qs?x?noR'?s;³™ÚÊ?x?noR'?ï¾Ù͙Ùä?€ø
#Fý?€IŒª¦ï?€ø
#Fý?ïükgpì@?0֩Ƕê$?<¤Ä	'
?0֩Ƕê$AGN4FGL J0931.9+6737?èÒ2"®@Cåwž™À9õ*8¸®2À<Œ
¨y0@¦Pç}@ïw݇/?²õçMVŸõ?¦ã,Š¢…Ñ?óŸÁ?/Á@
¡–‰ÄºZ?ïÿ·ÀÌ
Š¿â¿a!-!¿å1ß«Ì¢¿âß5…¿älɌ¦l¿ïmŸ`=AGNrdg3FGL J0931.8+6739NGC 2892?ïþPêm
‰?ìHTKB?*ñX0A:ä?ìHTKB?ïõødL¨?Uôþ~Oƒ!?T7Ìd8	?Uôþ~Oƒ!?ïóí¡iØÈ?]Ç="©¦r?X$¼« á?]Ç="©¦r?ïõìg(à??Ç]+nëe?T'2ª??Ç]+nëe?ïýê5=?)OzI]?1⩋v$?)OzI]?ïÙpô>%?uhˆÒîô?sG…¼¡=H?uhˆÒîô?ïìǙ\2?r<qTø§?c8fwÒû2?r<qTø§?ïçÁÍÀ<Ç?V8´	Y…?h>2=‰?V8´	Y…AGN4FGL J0932.6+5306?ï¥væ)@F ÇŸfb5À9¡®×€*À<‹íóŽ¶@b9®øP‰@/ÜÌõ?¯S¾Ãõ¶?µBJ¨DØ!@Â;C¢ìÿ@†Èg¸K?áÍaýËó3¿ãÑG»€t/¿æd2Dꁿ炞«QR¿è7·6¿ãÐ9h×YïAGNfsrqS4 0929+53?ïþ͏â®?‰'ioíç?#&ýÍÈXî?‰'ioíç?ï÷Gå¡|?RHœ7îص?Qq΀wm?RHœ7îص?ïïŒ<¹Ä²?]aK¤5*b?`sÃÀíù?]aK¤5*b?ïÿvXÝøÕ?æO˜?4äжC[?æO˜?ïþ"tÌä?&ž}‹ŒÐ?.ǵÐRŽX?&ž}‹ŒÐ?ïÙ"
8?xåênâû|?sq=·Ê÷Õ?xåênâû|?ïÐƱL5/?}Âå¯ú‰?wœ§_dÈa?}Âå¯ú‰?ïÿø—£?ærBn?@ôtâÙõ?ærBnAGN4FGL J0932.7+1041¿éBe¶ú8Ò@DIÞ½çÀ:ñŽd²1@À<ŸN"
@ /¤¨ìGç?ûüÇÓ¦Ü?Ì" 3§!?жIÿj.@S¥Ýt»@GmÑi¿Œ?ã[}i¸*~¿é˜¤ Üš?ÐÓۉÓÿ¿ÍøNñ¿âÝø©Êi¿ïÿ£^ilÖAGNbllNVSS J093239+104231?ïø‹í^'²?@;+Ã7?MÐK-îâ?@;+Ã7?ïéP"ÿ?f;ˆäŒÿO?f篦6Z?f;ˆäŒÿO?ïØÔñ-X?k7B
3Y"?s•‡Vmk?k7B
3Y"?ï£È §?eæܗùV?‡:<Û¶F9?eæܗùV?ï÷Ab ß?GYÁQY?Qó}šóQj?GYÁQY?ïºy§Ð'Ô?€–YÏNdA?a–HE$?€–YÏNdA?ïۊ#s¼?}:'FïÌ?~2:ó•Ï?}:'FïÌ?îݲ {¶?‰ìo??¢$ÕôÕÇ?‰ìo?AGN4FGL J0933.5-5240?âM'>÷ü¿åÇòÝ؍ËÀ:Ͼï"xÀ;È$g¾U;@!B<¨§Ôp?û´ò»sÞõ?Îß$}¸½v?ÑhEƒíµÑ@½ÞÎW@U›ÛhF?ïeû7Cc¿é MÈ௿ÜÒýhv¿Ù6ªK˜"Ç¿Úó­¡¹M¿¿çÓșaeAGNbcuPMN J0933-5240?ïìýMŒêx?Z[L#Ž?c²Ÿ‡P?Z[L#Ž?ïË&
(?(i͙fq?zlúöù?(i͙fq?ïr¯Bg?Š¯è‡à«ô?'¼Ê³o?Š¯è‡à«ô?ï´%<‹²·?da±'V*ä?'ö°â'²!?da±'V*ä?ïüÓãõç?y'¸t?~!–DŠ?y'¸t?îHwÆO?³Kåw6Äí?«x'³ÿ?³Kåw6Äí?ìÖ^+'²?¨
z5ô°?¹MXÉ«ì?¨
z5ô°?îz<]Ð?"&3'Ëìt?¨^|<Z‡?"&3'ËìtAGN4FGL J0934.3+3926?䙎ˤ@GÉ-ÀÊ`À:-ŽÚ"ö¥À<‰ì©&¥@}ÈoEF@i3]$žE?·3Øõz?Ž8èÿ³T?ÓþzÄÂ<@É"ž:"$?ïýqåöi~¿ä\u¡Â²í¿æɨnZQ¿â¹Ùె¿æöJ²È¿ïÿø¨ó©°AGNbll3FGL J0934.1+3933GB6 J0934+3926?ïý" 8D??(z\"äÔ°?3Úüp‰ˆ?(z\"äÔ°?ïöoVÇß?Ràý'ÁÁ?S!Sºw¨?Ràý'ÁÁ?ïé<û;¨«?qí‹k¨úq?fçzœð?qí‹k¨úq?ïé4ƒY*-?QkуĆß?fË|¬U3e?QkуĆß?ïý8挣?15ÅÈ@\ý?7:
v©:?15ÅÈ@\ý?ïÕEQ÷L0?tñc˜øR@?u]W9 ?tñc˜øR@?ïބܷë-?wýÞi	µ]?p½'šk{?wýÞi	µ]?ï·hAæ\ô?n–œkyÊ?'%ïyHý?n–œkyÊAGN4FGL J0934.5-1720?ٙ۱Ÿ¨Z@8ÃF4—·AÀ:åV"tnÀ<__á'@ 됚—?ÿ%"ü|?ÇÂЊ¢H?°³¢?–ª?îïŸËm@­Åñxô¿ÜÈ'ç%"¿êõŠèü®?ïþ@!Ù¶¿è³2ÇÓi¿Û,kãþ"¿Ñç6žË2AGNbllRXC J0934.4-1721?ïþ£©é?"º™ÒóO_?.ž'™Åʝ?"º™ÒóO_?ïðàY`]R?_Äg‰JO?^?MÅöè?_Äg‰JO?ïì¸G"£é?`­ÅÛùÞÑ?cG¸W '	?`­ÅÛùÞÑ?ïã	]²ôÆ?W‰ëìl¹3?lö¢)OJ'?W‰ëìl¹3?ïüÍ`ùó?0•-È;?9"÷ðžz­?0•-È;?ïÉKW0,\?}*RßTõŠ?{ZTZ+aÜ?}*RßTõŠ?ïì4$þ?l4ÆìóÄ?cðú›Àyþ?l4ÆìóÄ?ï"(wS¯¼?ƒ!º«^Q?Šõâ Å=$?ƒ!º«^QAGN4FGL J0935.3-1736?æOvl@8¹'^éšcÀ:GäB4WöÀ<2Ÿèh3Æ@!mQ³¦á?û®Ð³Z§?ÄoH7QOÿ?º¢žA-?üG*{Ԍµ?ÿ·Æñ¬¿ïkÚ佄Z?ïõeݪj¢¿í†òÞ€é?Öª"XŸÔ¿Ô¾B%>}ê¿ç:R ß²AGNbll3FGL J0935.1-1736NVSS J093514-173658?ïû7Ä<…l?R›"^S²W?C î[>Ÿ`?R›"^S²W?ïã'r•ý?qÛþ"(?1?lnèz,2å?qÛþ"(?1?ïÊS-Ø?~¼õ/ÆÝ?zÖi Z‰~?~¼õ/ÆÝ?ïÛSø¥?[ä	|šù?rVÊ<])?[ä	|šù?ïÞðÝ•a?rĦ0€yV?p‡'bH3?rĦ0€yV?Arð?ž®ÐÜ}¤.?ŽWùóà?ž®ÐÜ}¤.?ï5bœq)'?•5%,³‡ï?™S¬qÚÛ%?•5%,³‡ï?ﻕp¦?'§E8JG˜?(ž"1#.?'§E8JG˜AGN4FGL J0936.3-2111¿ä.¬QÐO@6už×ÆûÒÀ:¿YHp²À<iéæ¹@ é#mîE?÷ d#–?ǚ¶Äø˜?ÔÛ:£¿ã/@¢HåL"@E`í²v¿ïÿýF\I?ï÷{+ðHÓ?ìäS äQ#¿Ñؗü`Ž5¿×<ü_·u£¿æåÂ!øùAGNbll3FGL J0936.3-2114TXS 0933-209?ïÛõ‡h?wnm{#?rwO/ï?wnm{#?ï×Ø>E
 ?|š¹ÈlÐ?tàÜËá?|š¹ÈlÐ?îRö>'"?›ô>€É]?§
К`Á?›ô>€É]?ïđÞþíJ?fÝNíU?}·rÊêù?fÝNíU?ïÆViKј?xy9t+?|ÔËzc‡³?xy9t+?ï€ÛÑ2É<?™Oa=çÕ?É¶½Lï?™Oa=çÕ?îJ´·µÂ?¤I¦´Ÿ?¯KT¸Ð&Û?¤I¦´Ÿ?ïgP\Êí`?"¬Q*Š°,?"ôdê†?"¬Q*Š°,AGN4FGL J0936.5+1847?äæ™/Dç@FR  ô×®À:®4|ßN°À< …S'wŒ@ÁÕh|Á?þ@¾kàùª?ʊÄê€;û?Ã*[]É´¿?øJÚ3½œ®?ù¥HÇD!Ã?ë£t'ˆÜ¿ê7N€–"U¿Õýu‹¿ÜžŠD<
¿ëP.Ë¿ª°#çF¡AGNbllGB6 J0936+1850?ïõÈ[Emj?S	9s÷ò?ToI‹"¬'?S	9s÷ò?ïÃû5§?i0:óU?~eN#$£?i0:óU?«üj?'bÈ- #?‡4N'?'bÈ- #?ï
qSf?D÷°˜?ž½.PÅP?D÷°˜?ïÔ¦ï–.?tJ´õ毡?u¬ûì#?tJ´õ毡?îèL²¶ 8?£üôr­?¡{4ԝü€?£üôr­?ï|Û]^Tõ?Œ‡»ÍUp»?d"PÅÅf?Œ‡»ÍUp»?ëÌ8úaI`?£[6t•¯þ?ÀÏzځ?£[6t•¯þAGN4FGL J0937.1+5008¿ä†²?i½@GVºI<‰ôÀ:?'Á^ÁÀ< *#¿ø©@ GÏ!É@z䢬h?ÁS¬åÑ«"?ƒåä¥@+e>H:+@
žÄ½B?í´®"%â¿âÀ_×,v¿åš9҉¥0¿å݅TÖ¿ïññ\Ï¿ïÙ§'æøAGNfsrq3FGL J0937.7+5008GB6 J0937+5008?ïóõîâ©á?RÌÀߗù[?X"¥à?RÌÀߗù[?ïôÑ7."<?TtÍÖã­?V]'lè.?TtÍÖã­?ïÜòÓ`?h äJo Y?qð±´–?h äJo Y?ïÍ7—à ®?aö¹IÖw?yd4/L×?aö¹IÖw?ïç–â°
ú?d)Áúö¨¬?hirN'?d)Áúö¨¬?ïÔÚN"a=?t½~䬠?u'ØÆqz?t½~䬠?ïj5	Ä?è5·[œ??'¿þ =ÿh?è5·[œ??ïV}a÷ä?ðØÉò?•0S¿K®?ðØÉòAGN4FGL J0937.9-1434¿î¥ÒPU"@;7Ffìž#À:v^$x…MÀ<o»^æ?e@ 
Õö›þ?ýæD·%?Äú`XÛ8u?Á¤÷Ãpƒ?þXˆøa¦
@
ä"¬¿î¶Ãvö?ï÷uýÞÄ¿á"&ÈÁ¥Q¿à8äl-P¿×oXz™¿êá´N_ßAGNbll3FGL J0937.9-1435NVSS J093754-143350?ïÿ*)k«—?tL—§	¥?ºØ"¯P?tL—§	¥?ïõ»2ñnî?W{,蕧?T‰š- D¬?W{,蕧?ïí"œ{åî?r­oëo'?bÝcCj?r­oëo'?ïüëd"Ðv?#^QMÕ`?8¤ÝQ'õ?#^QMÕ`?ïý¨KQü¼?-Vh¬gê?2½£L‹˜?-Vh¬gê?ïÒr
c•Ò?}°ÑüÜê?vÆù>fãO?}°ÑüÜê?ïàA<q†'?}8C*€c?o¾Ã Wf­?}8C*€c?ïö§˜%‡?Eړæëå?R°Ï»öƒ?EړæëåAGN4FGL J0938.9-6403?␚®†T‡À!AMµ•x£À::Þ¨—c^À<;0µªq@?Ôó@@˜Ž¼ÆÅL?½ÊA¤åþ?­â~ðå ?ðXÑRm‹@éØÅ~yÙ?îˆ|:䝿äžr£hû¿áV™y¹*¿çôÀfŒý¿Öý'aĖ¿æµ¾§6AGNbcu3FGL J0937.8-64071RXS J093850.5-640334?ïýº‰q‰?%
®À*Xr?2+³C"³÷?%
®À*Xr?ïïùC'Ú?hùé,(Mä?`¼'ˆÎ?hùé,(Mä?ïôªÓ9Æ?[Ép>Þåb?VªYè¤"Å?[Ép>Þåb?ïùT…xþ?12¥jBt?J­ê½ñ9?12¥jBt?ïú
evÚÛ?=¸˜»<§9?GÊky-?=¸˜»<§9?ï¹Ì
£ñP?™gIv|Å4?Œü',Uþ?™gIv|Å4?ïôwR5Æ¥?d /ªƒå?W[{µ…Ä?d /ªƒå?ïâPYߚZ?[;ÆÑÊ[X?m¯¥á,Öz?[;ÆÑÊ[XAGN4FGL J0939.3-1732?ï¶=ñŸŒo@9yØ¥H#…À:
tÓ³¬À<Yõ2F¤@œ' PíÙ@'%IÆ?¼µ¿êç!?½Å°"òô)?ÿη«c@ÙÛ]3a×?ïýCWm¥¿å©?Êjå¿áÒ¯')c¿äKùӖª¿æuQ@9¿ïèÎ?ézAGNbcu3FGL J0939.2-1732TXS 0936-173?ïýøÏñ*¶?"Å[b
?09~ÓÀVj?"Å[b
?ïôHvç=?Z]=ëm?WoÉ¿Ž?Z]=ëm?ïò,æE¢?SÙ<R†×•?[צ¤'ê»?SÙ<R†×•?ïûybí`?)Aì¤_(=?BteoÎ?)Aì¤_(=?ïý§…7o?,}9."0†?2ÃÔÅöÒp?,}9."0†?ïÓñdTO?|Eeæ¿â6?vM»ˆ‡?|Eeæ¿â6?ïæÙ:(g?r[¿E \?i&øÙhœ?r[¿E \?ïôôʨìY?A B<t?VjBó~j?A B<tAGN4FGL J0940.0-2828¿àԜÏÙò@1éi ­ŠÀ9ùÓ°ìœvÀ<3ÅìÞ»@z[±×~@£ŽDÑÁ(?¸f¸³?ƙ˃ ±P@Mí®Ä¤	@Euà¬Óˆ?è]ÿÅGN¿ä` CAs¿å"—Ú|¸¸¿äy;.ª7¿ïþ—J4¹?Â<:˜Ø(¡AGNbcu3FGL J0939.9-2831TXS 0937-282?ïñña¬˜O?]œ|M²~?\<ØIÁä?]œ|M²~?ï틖'6?iDÁ)CXå?bti´þ'«?iDÁ)CXå?ïÃÐ&üø?x>œªéuÁ?~}—èaü;?x>œªéuÁ?ïû´w§''?,CâbÛ³?A. ãDu?,CâbÛ³?ïîdØOj?^t0@Gm?a›'ÙÐÐÄ?^t0@Gm?ï'öž¶L?•°³pîI?‹BXwâÐõ?•°³pîI?îì€Î5qk?˜Ùìs?¡7ó ôlN?˜Ùìs?ïî}«É¿I?O‰Ò"F?a'TÆW£?O‰Ò"FAGN4FGL J0940.4+6148?æ|(Í~£t@Eš:э%îÀ:ž:'ÌE¾À<œl%Ã(@ ÿƒ'ǁ?ûþ FÇd®?¿[äØ1Yê?²ùÞÓµtA?ôʇx.æ@jk5Øÿá¿Ü¡]Þ,›"¿íNj¼[f¿·Ãñ®¿ÛiÝk폿æx`ˆ"?Ç7¿)ÌAGNbll2FGL J0941.4+6148RX J0940.3+6148?ïÿ=mÉ?"zTÎ/?N«Óì?"zTÎ/?ï÷YhbP?QrpxI¦?QÅM!|ï˜?QrpxI¦?ïútƒh2w?69ÝÌÖñÇ?F-òœ<?69ÝÌÖñÇ?ïôUF¥Î(?C?êæ?WUsÙ?C?êæ?ïþê¾û'ÿ?ü>sWçæ?!TKŽ?ü>sWçæ?ïÛS×Ý:ó?tz©¦Aq´?rVô…ι?tz©¦Aq´?ïüîÏ<N÷?Pcmëoj?8‰‡|FÍ?Pcmëoj?ïÞø#pP(?^ö­!j?pƒîf{÷?^ö­!jAGN4FGL J0940.7-6105?ä¸0
À!)Es§˜À9èy§‹Ê¤À;ڽۘA«@—Š«j&@æc[ïêß?ÁEj˜?Áâò=ŸÀ@;†Eÿ¾'@	C\($¿ÝÇkäՂ(¿ÓENJm¬¬¿æ}å=ÜÚa¿ç¯žˆì£,¿ïicÁpx8¿ïÿú@ùDzAGNbcu3FGL J0940.7-6102MRC 0939-608?ïúçœr<?9êi"¶…?D`õ¤ÁL?9êi"¶…?ïèÆǓì ?mXÚZ֚"?g98šÎ?mXÚZ֚"?ï§Os@û"?'8úRƒ
ô?†,#,Qƒ?'8úRƒ
ô?ïÚú'WÛß?WX˼Ž?r'¶ÄóȎ?WX˼Ž?ïÛ÷¦ƒý?rês­H€?rq`©×?rês­H€?ïf˜7Ľ_?¤¹"çYž?",ùhT'?¤¹"çYž?ît£Cw­? ÂËV«€?¨µÎûȅ7? ÂËV«€?îöÆ&P²Ü?Œ¨uÄA&Ö? "œ¬ <?Œ¨uÄA&ÖAGN4FGL J0940.9-1335¿ïþL?QW@<lӝ¡fÀ9œÈ\ûƒ™À<'Kžd¶@üËÙ1ß÷@g'ûÈbÛ?²z|öê?½iIśÖ
@‰—Þ®v @¥o;¢?иœ>9¡Œ¿áŸ=ب£¿äNô‰u_¿èWÿ›V2¿çþîк˜¿ïùö€û=#AGNfsrq3FGL J0940.9-1337TXS 0938-133?ïýëm¡Ä?0@ʈG<'?0¤'ÝóW?0@ʈG<'?ïõ]ùv?T8Qóð)­?TýEf—³Ã?T8Qóð)­?ïíDÀ¾‰?ZÆIü@?b»?aŒÞZ?ZÆIü@?ïþuj –_?šä¢Íd?(©_ý'Då?šä¢Íd?ïþ¥ï,7?$TMˆ†?%¡>cUà?$TMˆ†?ïՋ™B?z.!(³K?u:3cIó^?z.!(³K?ïËm°ÌTò?zH
çTÚ?zI'£to,?zH
çTÚ?ïüM…¼?/U""YÉe??&œÍ–^?/U""YÉeAGN4FGL J0941.7+4125¿â×XHÚÁ@Hp}€^_1À;@·E|À<º¢ô§@£Nçï'õ@q<ƒ>?מý0ÂÁ?å
ƒç€­:@È[TŠœ@
eBŠ¿¿ïë"ÌÐþ‹?ïÿì´É È¿æ/ñ)£gy¿êOž£Ä•Ç¿çõ2F¤¿ïü¾â©WþAGNbcuGB6 J0941+4121?ïèºy÷?qÏ,y"%?gE÷ÅA½¸?qÏ,y"%?î®HhW4ù?­» ΒÛË?¥y{h—s?­» ΒÛË?îb êcê?šÔñDÍÑ?©ÝñYÁ^Ò?šÔñDÍÑ?îQšù…?'4Hf^g?ªïè5°?'4Hf^g?ïÇŸé¦?ˆm{Œ	y?|p/ñôS?ˆm{Œ	y?è‹("ð?Ï䐮
™ò?Ï¥Ó_t?ÿ?Ï䐮
™ò?ì¤J¯ü‡{?©c/Ýåº4?ºÝª€Ä,?©c/Ýåº4?ލ
jÝ՚?À¤Æ7K4¡?à¹yJ'3?À¤Æ7K4¡MIXED4FGL J0941.9+2724?ï¯CãÀÀ`@HëC,¥À:<éhSÀ<Œ_Æ94Õ@ûˆ÷5=@-'$ZR\?¹ùÛßËhZ?¸r*rD?ø§{‰äð@	É0àóu?í ¶ž¸¿à‡)T ¿å:óṘè¿é£L Â'Ç¿àn—Oß¿é$Læb AGNbll3FGL J0941.6+2727GB6 J0941+2721?ïþ×/[b?ðÉ#è#$?"ŽNrí¥Ã?ðÉ#è#$?ïõ|'çg?TŒ1(ý\Z?Uچgs?TŒ1(ý\Z?ïôÔê":?I·ÍÂ=ÕÈ?VWÌ;›Õ?I·ÍÂ=ÕÈ?ïï3èB|°?Gß×êì?`Ìé~Oæ?Gß×êì?ïýÖ¨ÿÏ??'UN?¼^?1J¹fÇé?'UN?¼^?ïÊEj\.?_Ø…ò5?zÝJ²LŒ)?_Ø…ò5?ïì2[z'±?h"¤ÿ§.?cͤy·j?h"¤ÿ§.?ï´ý'aé?p·mz˜d?'À›…få?p·mz˜dAGN4FGL J0942.3+2842¿ÇŒöE¦@H<'RT`ªÀ;D€'q^èÀ<È<){úL@ ¿›7©d"?þ,7«gø?ÆViGt‰?‡ºhµåÄ?Å_<¦y{í@Pò‰ø¿ãù`ÃdC¿àÆv;Ƭ¿ãÈßëb¿×:,âMf¿á°@¿ã°>¿ÔýAßAGNbllNVSS J094223+284413?ïÿ(»C?//É%Ò?zþd¦ž?//É%Ò?ï÷Bà-y?RávÖ·¹k?Qz?NT?RávÖ·¹k?ïù
ÆDÐó?\³¤YÈÃ?KÈç<s#'?\³¤YÈÃ?ïýВ¡z? ý5Ÿ¯9?7}o¹k²? ý5Ÿ¯9?ïÿ $Á3?1ÑVç?{õ™Oqµ?1ÑVç?ïÙùH«À?xË$"+aÅ?s|R»#Û?xË$"+aÅ?ïûnêÞž?Vö¥6ƒ¾?BDU	ÐR–?Vö¥6ƒ¾?ïõO6ìG´?F$âý¤Êâ?Ua'nèx?F$âý¤ÊâAGN4FGL J0942.3-0800?±í™ÁŸ­@@'1]pŸÀ9—2éaX
À<^6=@e¬|`C@ç¡di6?³m0/Î?Âu'ÿ ±ü@AÁÇ@£$fˆ ¿ÁgncµÜñ¿Õû"¿e=¿áƒ^nË:¿ã@*'zÁg¿åb¼ù2±¿ïúÀZ΂¯AGNbll3FGL J0942.1-0756PMN J0942-0800?ïûÍUÞ®Í?:vâ£YŸC?@ʧí‰Aë?:vâ£YŸC?ïóLêÙ ?_³ºÀ¥^?Yf*	2?_³ºÀ¥^?ïĨÝÉ
>?}8ä|.¸D?}«'¼0ê?}8ä|.¸D?ïý¿û"?"4¦ªî
Œ?7÷8yÏ¿è?"4¦ªî
Œ?ïùé![S?D4:PÜäÁ?H[y SþZ?D4:PÜäÁ?ïÃÊ©¡?"´ü´
?~ýù®ïÐ?"´ü´
?ï~axã8?Bµðÿ5?=³Öö?Bµðÿ5?ï÷Pä‹$??v~ÆBúJ?Q^7£oX@??v~ÆBúJAGN4FGL J0942.7-2028¿îUö^Áj@8	WG²JÀ:Ö½A>Ž±À<'›Ø'@¥:=h–A?þ£ð4°áµ?Æx»þsc?¾iAžA/[?ø²'¸#È@ÿŠÏ§G­?ïîá"Úíø¿ÒwØ¿cm¿Ó:4g¾€¿áÄÏ9°%¿ÝÀ¯óx2A¿åÍôIéXAGNbcu1RXS J094237.9-202720?ïþT­ã?t¡'Üs?*¿†U«–d?t¡'Üs?ïòXŽÉö?X°í…Ãe¨?[NãŸðsb?X°í…Ãe¨?ïöq+;m?DdnÄ'šR?S©ËX§?DdnÄ'šR?ïíÝçYôq?@«ù3ù¾?b"¯ªw??@«ù3ù¾?ïûtóqý?Bw>"?
?B,1N+?Bw>"?
?ïÉT?GhŸ?Ož6÷5?{Uàfš"I?Ož6÷5?ïíºìS?pT5ñXd?bEñ€P<l?pT5ñXd?ïÀB&"èÌ?g©.s™w?ÞìÇÚmÌ?g©.s™wAGN4FGL J0943.7+6137?æ -r‡‰@EÑ(9-ŒÀ9ý,ðùÒ¿À<q
À²ã@íúCR@Žm=ðüW?´ÇV2ç‰?Œ.·´è?Õ¿~°Š!@Oš¿ßS?ë]F,4;q¿Ýq¹`‰W­¿éOt.©6¿å¹ôMDVq¿ïÿøãú?íÑØÀ  AGNbcuFIRST J094420.3+613550?ïÝr@((?­'ÔɃ?qFßÕ>"•?­'ÔɃ?ï÷÷6ǁ"?Pî&6g'?P'›ßA¤?Pî&6g'?ï¶óM®ÎN?'búØÅÍ?'C,ž›@v?'búØÅÍ?ïý¼ü³Ã?"ô2 ŒN‡?2"él?"ô2 ŒN‡?ïü¦KP,á?=פœÎY?:ͦÕ(?=פœÎY?ïÝI9YèÕ?q\‡' t?q[cR[©¶?q\‡' t?ï™7OˆºŠ?‰hŸ˜å~D?‰²,!@ùb?‰hŸ˜å~D?ïøX®dNV?C`¢È~ç/?NGµ(¿?C`¢È~ç/AGN4FGL J0944.2+5557¿Ë…»¸Ÿ»"@FûŽ\NµpÀ;q¬O~ÃTÀ<üóæIî@—wȹm?ý–¡G
Ë?ډµ@>3—?äûë~Õp@—ÕÄÃ?ñðtY™#}¿ïýv:ÂÊ?ïÿÄ}îB¿Þ¿EE•6¿ámžÔký¿ï°B¿êfì"¨vAGNbllNVSS J094441+555752?￵¹Âb?º65³Ît?€˜‡…œ?º65³Ît?æ®Â2I?ÆB—n
?Ò¢{›èåm?ÆB—n
?íËy°?¡ä…"î¨Ù?·i¤3év?¡ä…"î¨Ù?äI)Å~ØV?±§Ÿ‰?×m¬uOT?±§Ÿ‰?ï$iàÞŽ?™'J÷'K±?›rÃÝ^@?™'J÷'K±?ÎFúê†4ý?Çr¥µ0Ï?ènAE^rÁ?Çr¥µ0Ï?ëKÌ"\?ªz7˜›?Âӌϱ®Ž?ªz7˜›?ÉÔ‹ú
'?²›55wù9?éŠþ]|œ?²›55wù9MIXED4FGL J0945.2+5200?ä1|½sq@G´"ÀÀ:YôNñ՛À<•Ìe÷@»MôU@Üʵ›?ÀÊóÙ¬T?ÁÛÕ~L69?ú˜¸É	Ê@[q¥ß£¿Ôlbñ¼Æ¿äˆ ËQ¢Š¿éx° œB@¿í•Œßvó|¿ïú¡†Íäû?ïðÝî]@MAGNfsrq3FGL J0946.2+5209WISE J094452.09+520233.4?ïýÔàB™?-ò®ªŸ?1Xýoyâ?-ò®ªŸ?ï÷k¼'–@?Q'—PôX?Q(†nà³?Q'—PôX?ïÝ/ý¬?rƒ$ÄÑÇÜ?qh=ªõÕ?rƒ$ÄÑÇÜ?ïüçléÀ×?))%	4‰?8Ě=ÌEì?))%	4‰?ïùñ,ÊÛ¨?H¯¿^'K?H;KÎâSM?H¯¿^'K?ïÛA¦µÙ?rµ}ìè?rq_—φ?rµ}ìè?ï¾¥q?€·—üùtÒ?€yûFcÄ?€·—üùtÒ?ïìó͆tè?WRcÜg¯E?c2Ê'{?WRcÜg¯EAGN4FGL J0945.5+4635¿è=®ün•@Hf¼b~À;åác\ƪÀ=—^Uö­@!ÏÎ_IÀ?þº©êIµV?ÅŘ•2¿¸9ë‰%ƒ?í–?aê«°@!¼:®Q¸?×A¦=–ä^¿êWvßZn¿Ö·¯™¶¿å®ùèŽÊ3¿ÒS^a_@'?ÍãEµ÷AGNfsrqB3 0942+468?ïþ'€ùî!?òýwû­°?&çïR£]?òýwû­°?ïöcÞï©?Vë‰tâæ?S8B"ém?Vë‰tâæ?ïòîhÂ¥ñ?cӟû¹™q?Z#.%}Î?cӟû¹™q?ïüaIhv?+r&?;"óœ,"°?+r&?ïþTl?#WóäŽa²?*¾³ó1T	?#WóäŽa²?ïÖ­ƒ±Oï?vسŽûïo?t©>'X«?vسŽûïo?ïõ­"mý×?fF`<Bß?T¤ØúÉ•?fF`<Bß?ïçs¹'‰?b·xۓ¤	?hŒFPžý?b·xۓ¤	AGN4FGL J0945.7+5759?áYÆDóO@F±3 @|ÈÀ:Âð\À<'*¢jùs@[êæhTR?ýþŽæ¸0^?Ãëv?Úá?Í5³Ö†´å@üŸS @
…ÊúåŽæ¿¹)LÕpµJ¿¼µ,òý8%¿ØR'_js¼¿Ù;}8ºÝ¿épà"&þ¿ßVóé	AGNbll3FGL J0945.9+5756GB6 J0945+5757?ïõš™HæÏ?QB(6ßt?TÊÍÈè+?QB(6ßt?ïô÷@hÐÏ?Sáø™Ï?V]õ?Sáø™Ï?ï½´©?~ñ?x'Fà'y?€'Õ£¿Ô?x'Fà'y?ïïW"Ý[!?BƵãrÀ?`¨zòŠW¥?BƵãrÀ?ï×nŸM–>?s-Ud£%?tH°F¦üÝ?s-Ud£%?ïÓU$þÔ?u%ÝGãÖ>?vUm"€ù®?u%ÝGãÖ>?î
t¶úí5?¦6'5L]¿?¯(´'ú§?¦6'5L]¿?ïÄgùìô?fÃ6õ'G?}Ì)"^µ?fÃ6õ'GAGN4FGL J0946.0+4735?âÚEvµF§@HW<ÈóÀ;ŒDÄU/À<ÝêPkR^@ ¯7eœè@ËHZ⤥?ÁY°àÝûÉ¿¸ö·Au@I?ùìÅÛA?óc-+²5r¿î~¸—·¿bø;v´Îe¿ê½¦îí¿ë_:øúRA?Þ]JÿÓ?¿Þ3xgðª"AGNbllRX J0946.0+4735?îbøµ»?Çx|"q$—?©Ö |…S?Çx|"q$—?ï¿ÊåZÑ÷?"=ŒlNK¬?€
F£Ì"+?"=ŒlNK¬?ï8	ªv®?•ë-â¶?˜þß® Æ;?•ë-â¶?ïö€v;?Ml{O•ã+?Sü{к™?Ml{O•ã+?ïX‡ÛMy?Ÿ¶jZÍ‰?"ïžäöÔ?Ÿ¶jZÍ‰?ì©áõAÏÈ?Âñ²Õæã?º°ðUñÁ?Âñ²Õæã?îŠThsB(?¡¬ëZ&s$?§Z¹wïö?¡¬ëZ&s$?î¾ÞK"è?¦á -,j	?¤IRFƒ?¦á -,j	AGN4FGL J0946.2+0104¿îúz[!@CH
|ZÄrÀ:¶ßh°ÄÀ<[@dtß@!T)΅‰—?ü‹'™Ù?Ëùwœn¶?¾Ö?;‡?ô›ƒEW"@¤}M]«Ø¿éo»^g"¿ÝÕÿ™'Ú¿ämð‰Ó©¿Û'/'y—q¿¤ûg{¯¿é˜=‹ü£AGNbll3FGL J0946.2+01031RXS J094620.5+010459?ïþTTÂ?ûEs±Y ?&ú»Ü]m?ûEs±Y ?ïótJ™p?Y¶¨½µÂï?YjoªpÎ?Y¶¨½µÂï?ïòHú´€?^¯¼°œØÐ?[Çmµ`¯£?^¯¼°œØÐ?ïøÚ)à+Ø?7©‹?ÀÉ?L—XñI±?7©‹?ÀÉ?ïûi4ni?D'»Î%
?C'[:^•Z?D'»Î%
?ïÂUɊ¶?"O¤g"ÇÆ?~Õ7ËØ?"O¤g"ÇÆ?ïéS‰Gš|?rV	ˆÕ%0?f¬våÀ[Ì?rV	ˆÕ%0?ïÐÿçl$?n¸V7'k?w€t#§EÈ?n¸V7'kAGN4FGL J0946.6+1016?×=8pÅ÷@E·<³åu:À8†'M!À;ק{¬]@æP4JàN@ÀÐ$p!Ñ?Ÿ|/Ùêö?´Û³@^çßwÊ<@´Çç4×ù?ïо"$哿àð´"†è'¿æ—ºÁÝZ¿çlÏ¡"c¿çµ:uFÔ¿ëëJ ŠAGNfsrq3FGL J0946.5+1017TXS 0943+105?ïý¹TÜ•?$ó@õ"?25WµžQ?$ó@õ"?ïò%d¤?_Ó@"T÷?[µ8[éN?_Ó@"T÷?ïÙږ±TC?w‹ã fN?s´šGZ°?w‹ã fN?ïüH&gü?/Ɂ7PåÓ??ÅÀ©ðAž?/Ɂ7PåÓ?ïþ´«:MP? 테kè—?$µNØây? 테kè—?ïͅµÈ4ž?>¨Þ¼R?y=%"Äé
?>¨Þ¼R?ïÉädÿg?{Ý@—Z´?{
ÍïqÈ[?{Ý@—Z´?ïöYáÑIg?Dê`nN8?SL<ƒèÒ?Dê`nN8AGN4FGL J0947.1-2541?Ó|ïl{@5Ý~Ë·úÀ9cf´iÿxÀ;Üå`A‰7@Œ•]õ©?üɕà§?°Xù:>?¶w%ü=ÿ@
'¿}Xñ3@
9¨…oÁ?ïò'x=?Пà·õ¥¿Ô¡â=wYÔ¿ÞgÚúâß´¿ÜÕÓ;{׿à 4éì˜AGNbll3FGL J0947.1-25421RXS J094709.2-254056?ïýžlÎE¯?,S3˜#ì?3˜ãß?,S3˜#ì?ïéÍlÁ©?cÿ&–¸­Í?f2"+½‡X?cÿ&–¸­Í?ïèŸÌÂœ?gqk[r?g`3Îð?gqk[r?ïÜn\mØå?S ²-5Ú?qÈѸ•mp?S ²-5Ú?ïûvd?8Ð,ßîð?B'òÉqߨ?8Ð,ßîð?ÆDي?"ñ
Ív[?ˆ×Î]›'–?"ñ
Ív[?ïÑ)ï£Í‹?~·Ä´CÎÀ?wk>—ZD?~·Ä´CÎÀ?u¦˜?tº+ݘë?‹•¼ìå.?tº+ݘëAGN4FGL J0947.6+2215¿Ðüœü®@HJƒ±ÐÈÀ:ðë€ìújÀ<´¹‰$@µE@ûZ~ї?˾_·¼^?Ðe)O"¢'?ÿý&g@Úp'ÉôU?á΄'Ai?Ðgâ<u§!¿à"Ä"ïï¿ã´zÆo»¿åˆ©©µ¿î•³€ y]AGNbllTXS 0944+225?ïü¨†F?4&0¹"??Ú»zÕ?4&0¹"?ïòPeX?\oð;."Ä?[_ݘD''?\oð;."Ä?ïÙ\"D^î?mª_-BÉu?sQµé4¼?mª_-BÉu?ï×Ò2x‰e?QùÓ¡ÃUË?tæÍZ5ˆ?QùÓ¡ÃUË?ïü<×KÖÃ?7/ñä*?>CçHö\?7/ñä*?ïÉû³âg‹?{>ՊÌz?{& ª2W?{>ՊÌz?ïµñ@A%?ƒW_ÚPƒÿ?'ƒ¯ïÊ­?ƒW_ÚPƒÿ?ïocóøé>?w=T‰ñ@?'xKÒM?w=T‰ñ@AGN4FGL J0947.9+1121¿æ­J•@F¸ºÇÀ;n'D:ÂÀ<›@'§@ »;'HnY@¢õ}Åþ|?¢#€ã•;¿¾Ìô9ù ?õò-å˜î@Ó£¬íßA¿ël™ñ®-¥¿æo"‡¹E¿éÍÝ~냿ÕòŒ–›¸¿ÕmË"°¿â=v:ÂÊAGNbllNVSS J094746+112020?ïþïãìè»?š½1Çç9?!¿Lï?š½1Çç9?ïóþ5ê6"?YғI—"o?X"(ÓH;?YғI—"o?ï÷²ÿq9Ô?U2PÕâs?PšbD‡ˆ?U2PÕâs?ïýÞ£+'?#¤ÅÀ?1¹âçm?#¤ÅÀ?ïüFå.Ž?@¬¹üÏk?=Èפ‰
8?@¬¹üÏk?ïϐ0 ?wÇP"?æ?x{óY"?wÇP"?æ?ï÷¨jJ?_έ,?Q¯Ah|?_έ,?ïäñR#tŠ?hU'ªI'?k®&H?hU'ªI'AGN4FGL J0948.6-0338¿Ñ;ƒêëø@B!ؾr–öÀ:ò6†¤ÊOÀ<|›U[|(@¤L9µ@R§åŒ·3?ÃéùÃÐϼ¿¨ªWVþêV?áõbLM@~á8>µÈ¿à0(QWáh¿Ùgð>Áܯ¿éÕ2ÌÛæ¿Ûà?:¨rz¿ïÿÙ3ã\[?ï¿xPs¶AGNbcuPMN J0948-0338?ïý¹£Ç'H?.žãœxš?22àœÂw?.žãœxš?ïõIE÷¹"?Y·^ÃFC?Ums՚G?Y·^ÃFC?ïÛ½€~•‡?lTF$8ÛÊ?r!?¨§ø"?lTF$8ÛÊ?ïü©K	à÷?&`«'¢w?:µ¥Ú`ÿ'?&`«'¢w?ï÷ß'v?XNiGw?PAòª;	?XNiGw?ïÐ0ØBªR?w@Ö¼<j?wç"ÑœRü?w@Ö¼<j?ïΞ觸…?´G
ԕ?x°‹"fŸ?´G
ԕ?ïâ›nŸµ?bd0È÷?mød'À#T?bd0È÷AGN4FGL J0948.9+0022¿áìCrpŠØ@C[¹pޏÀ7Û:,K¸eÀ;ÅÀ–]¤÷@~jM¦¦ó@Ÿ¬EmÈZ?œX¥f4?Å&J*øQ@$»`Iì³@O­·4¿ÑA¹my*¿äz™ú©¿éšñB¢çÌ¿êÐ3¿J-K¿îÇ·ºã¿ïÿ&¼,k™AGNNLSY13FGL J0948.8+0021PMN J0948+0022?ïCh͞ÙÊ?«R:ôy?—'æO"b¯?«R:ôy?쐭ðœ=k?ÀäŠG…ê?»z{¤?ÀäŠG…ê?ìȯWÔÜ?­íºl=½?¹ºƒ…AY"?­íºl=½?ï
%ʅí?"œß[ø?ž[^ŽzU?"œß[ø?î{—8Kî?«Ä9¹Ûç?¨FŽŸZ?«Ä9¹Ûç?ܼû ŸÈ?ÓQH¹ú"?á¡ø/°?ÓQH¹ú"?í"W
€?§¤{JÍ/?³]GG«ÿç?§¤{JÍ/?ä‡v,	ÑÄ?ÀÒxC™Ä?Öñ§ì\y?ÀÒxC™ÄMIXED4FGL J0949.0+4038?Ø-ÆTì)@I'½{ 1ÏÀ:{ôšq/îÀ<âž43@I²dkº@ñ^aµ&¾?º7U½¿"øæ'´?ÐðjÌ&´ @¡ïDÆÙn?ÎòŠ÷jZ<¿ãZK:õ†¿ë&qN õC¿ãâg3B¿ã{.¶Ì°¿áäúÀûÞAGNfsrq3FGL J0948.6+40414C +40.24?ïþ©a"?œ›HML?%f,ËњÃ?œ›HML?ï÷'î\i?R°- E\?Pú#ª!¤²?R°- E\?ïíÒÊxð¾?e-a1ói?b-5J–"€?e-a1ói?ïþWOƒ?Úô0¼l?/úŠÛ¦?Úô0¼l?ïý-°<sN?2$0÷)`i?6'€
Õ
?2$0÷)`i?ïÞi3폲?pŸ%¡‰?pËfI*Þ?pŸ%¡‰?ïäàwN–?qb·m‡d?kˆ›loü?qb·m‡d?ï÷a<þ/"?Ba¸¨7Í
?Q=†MØj+?Ba¸¨7Í
AGN4FGL J0949.2+1749¿Ø/&úüÇ"@G'«!ZÀ:Â㨱d'À<ˆ–&G'f@<ÁQnˆ@öå¥
ç?Å.Bž
A¢?Œ$P
Öϧ?ÂèyfkK@ø÷2Q
¿ì]ÒC.S¿¸¯ƒ»¶Ð¿è¸5›Ã?…¿àó›}Ê[-¿ìE¶ù%ñ+¿ïÿÉ–oAGNfsrq1FGL J0949.8+1757TXS 0946+181?ïýÎúú\¨?&=²¢m?1ˆ'dþN-?&=²¢m?ïö¯‡µ#?SeæƁ'?R òYFhÕ?SeæƁ'?ï̋>7N?zôê0¶…P?yº`äqY4?zôê0¶…P?ïþ¥:â?ÌkàG?/…©›¹Î?ÌkàG?ïþ`7ù«?(6k"Ó?)ü}‡`9ž?(6k"Ó?ïÕnÄ®Æ'?u¬Åâ$'?uHšÞ|È?u¬Åâ$'?ï՘Wœ–q?|‡bHÝD?u3Ô>_¦?|‡bHÝD?ïø
,\]?@
ð8]`]?M¿Ø=³Z±?@
ð8]`]AGN4FGL J0949.7+5819¿Æùy—àJÈ@FÝ]Ý*èâÀ:=çi0EBÀ<x5k×Í@Q¡?*bT@Î=EìÏ?º"tôô‰)?¶ûOþ+OË?ørÀF¬Œ»@zùdZr'?ÜÀÄÖ´,¿ãG(é-U¤¿çkÄߘl¿ë[î¾96-¿Þ¿â®‹n¿ïû›ûs©AGNbcu87GB 094609.3+583301?ïþì7ÝM4?
ì3!Þ?!<ƒ0ÛΨ?
ì3!Þ?ï÷È+'v?P•'e½Ó™?Po©= ÿO?P•'e½Ó™?ïñ‹Ý],›?J¼}˜Ø?\èE˜j5?J¼}˜Ø?ïû0Ÿ'¬?+®I€®?C=½7úý?+®I€®?ïþuÔöðj?"wáW#m³?(¢²¿†£0?"wáW#m³?ïÚýI
Ý[?tÙNѤkè?r[]"rÎ?tÙNѤkè?ïéÃΩúC?k@õ9ç¦?f<19)¤?k@õ9ç¦?ïèelôӅ?V‰t@@MR?gš'çp‹‡?V‰t@@MRAGN4FGL J0950.2+0615¿à£Fñœ@EFA,ðúÀ:Zˆàä±ÆÀ<n;è
šó@ÐÉéC?ÿ`_¼(:?Á ¥¼è~.?ÀØÉÛ*Þ{@9}I׺g@«ÕÄF™¿ïÈ͙{f©?ïÿ3¶>ì¿â¢çUåã¿Þs²LîÆ¿áG§~´ì¿ïûÇVkF AGNbllGB6 J0950+0615?ïüíòʖ?2ak@E€?9â'߀Ά?2ak@E€?ïîBÔC—7?`ðõsþ‹&?a½+à$¸²?`ðõsþ‹&?ïçræ…
N?sá"üù?hTw?sá"üù?ïÖ
Ž#nÅ?YԒ˜cY?tú¸Ö;YŸ?YԒ˜cY?ïó:êY?UØE²òÀ?YçùÙâ=Y?UØE²òÀ?ï¼üüóå?ºÖï%=W?€þ@ËiÐÊ?ºÖï%=W?ïÏh©ÈÌô?}Xi7£ó¡?xK«‰Áó?}Xi7£ó¡?ïDU`ã"?"ò‹{³O"?—~5\z¡©?"ò‹{³O"AGN4FGL J0950.2+4553¿ïÒ*òiP@Hß`|A™þÀ:¸7êRÀ<…Q(ÀB@ŸTÄ}s?ÿz"¯tÍ1?¶-z¢§>?¯6¨¢e?ؓÓ›fù@<ȋ­?ê;KÀ¿n¿ÑÄÝÀ$5¿å4Ô#&¿Ò¶´DÁ¿â2«ž~Û¨¿áÊFà!AGNbll3FGL J0950.1+4554RX J0950.2+4553?ïûP`ôB?9$íÐ4õ?B¾|à´p|?9$íÐ4õ?ï÷
À)r·?P¢Å¤ÓÌ(?QäŒQ:?P¢Å¤ÓÌ(?ïò¾fê?]#,]‰¦?ZƒÍšŸ}?]#,]‰¦?ïâ<ÿ€X?U\"ýéÕe?mÃ҂(B?U\"ýéÕe?ïõš§>P{?MŽ±Ò¬%?Tʱ'yW?MŽ±Ò¬%?ïØc†²	?uØW°Æ$ö?sÎ=6¿®?uØW°Æ$ö?ïïŒknõ?n,üIQ¢?`s"‹‹Ž'?n,üIQ¢?ï¶Kûoç2?lÔU}×y?'m$^)d?lÔU}×yAGN4FGL J0952.1+3932?ì–Çùd–"@I€Ž6FÀ;rð\À<Ø£oqY@!‰Œ{ÎØk?÷êÐ"¢§?Óå¿âÙ~Œ?ÌyÞýPù?ü5K÷OWV?ô ˆ­Ž¿ïÿÿ" 5•?ï÷‹Pb?í€ðÀÇÛ̿ӊi%¡_¿ÔÌåÄ—¿Ýx(Z½ëAGNbll1FGL J0952.2+3926RX J0952.2+3936?ïùš¦	¥?H(88Iˆ?I•fßç§?H(88Iˆ?ÚØÃ?"‡®›Å?‡¼T×?3?"‡®›Å?ï† 
´®?Ž/Α‹?ŽwüÆ!¨j?Ž/Α‹?ï
Ø "ß?†²F—F¶¦?ž¤ëüÈ3?†²F—F¶¦?ïúK¶•[z?@µPº2$á?FÑ%è$±=?@µPº2$á?ƒ£°k?¶†›£?§GGÁyvR?¶†›£?ïŽÈH"Õv?‹ã*¹vX?ŒMíÓëj–?‹ã*¹vX?í"KÿTUå?¤Äâp°³?¶í iÙ?¤Äâp°³AGN4FGL J0952.2+7503¿àãÒhJʲ@BŽÌ¼Õ,À;}§´æÀ<÷;«§¹@#2Xëÿm?ò:¦ú«,i?ÜHñáYKÌ?Ô¶VÿIh@¤m'Lž@7mŒöH?ïOÄÞì´õ¿á¶2 ä|¿ï¡±`_¼(?î»4ßZÃñ¿ª]{íñ¿Ì‡Ú¿Ô–ÆAGNbllRBS 0804?ïúË[;Bª?=x>ãñÛp?DҒÚUb£?=x>ãñÛp?ïõp«wC?T[v"ó û?U©ÕÑ):?T[v"ó û?ïÉÆ¿D­?uN¢dkQï?{ü2덡?uN¢dkQï?ïûŒ¬÷?;£¥´~Wí?Cèõ†—&?;£¥´~Wí?ï÷Óºª?PÒÌÚö"?QÆXœRÌK?PÒÌÚö"?ïÏ­ñP¡?z&õ¡{?x@)§Ã?z&õ¡{?ï­úÏñ?"¡¦h–¬?"LJû3º?"¡¦h–¬?ïë}9f©?cÄ8ØÿU?d'Ƈy­?cÄ8ØÿUAGN4FGL J0952.6-5048?ïõTEÛ	.@9¡vݬïÀ:ªî!±*°À<2kÛñ,þ@ rUãâ=!?ÿD*Lä'?ÎۂGB‰½?ËÁЈgB?ýIƒ×u.@	qÁpÎ\¿ï'Óa'jv?ïøx·¡Â]¿ÔìKî¿ØCe'Š,¿éý7%?¿È¡ð•©ÊêAGNbcuPMN J0952-5049?ïù‡v4g?Iì¾/<J?Iâ'Vª¿5?Iì¾/<J?ïجºÎ+?'~BiFÂ?s©¢÷ùb¸?'~BiFÂ?ïÆãàÉ?víñÉf?|þŽ%F/j?víñÉf?ïðJnåÎ?FœˆjqÂ?_k#Ñt³ý?FœˆjqÂ?ï÷2jÐQ?Sö¢¬8gÛ?Q›)ÛÖ]û?Sö¢¬8gÛ?îeÛ	./œ?³º•\†^?©¢Oi­jG?³º•\†^?ï5Ý«Á?"èDQ²‡ú?™D]r¹ë?"èDQ²‡ú?ᆱXÖ'a?på˜ÀìœÞ?€U)¹ Þ?på˜ÀìœÞAGN4FGL J0952.8+0712¿íÖÒ(p%q@E£?á—_-À:ñùÌàÀ<¢Jmâ[ª@ IúõÕ?þHåL"C?Ê¿Yòª?Ïã}h`'@]ˆ~¿"À@Ën–™	¿ìø0Èõ§·?ïõ>¦-ü"¿Ø"GNNí¿ÔžÒn¥Ð¿ïþa?ïæf¿QºAGNbll3FGL J0952.8+0711SDSS J095249.57+071329.9?ï½n§H?¬òÔ¬Õë?€¤\
78?¬òÔ¬Õë?ïÔ'´úÉ	?|õšÁ¢Ð7?uì%ž[ ?|õšÁ¢Ð7?ï1¼ð®Û?‹Ž"géX?™Èaè"6§?‹Ž"géX?ïŽÀ<z°?u´n"Ú®g?ŒOþðáT?u´n"Ú®g?ï"ãŠÜñ?`b˜ã?‹;‡.vϯ?`b˜ã?îæ,= Ÿ?«ôIŽ–?¡Ÿ=Ý?«ôIŽ–?íÍÍu¿ä?¡"ò0.}?±'"PO:à?¡"ò0.}?í<Ń,p?¥ñ(UAw…?·NҜÂ?¥ñ(UAw…AGN4FGL J0953.0-0840?ڡتß@@óO?Ù3ãÀ8d.˜™¿YÀ;n­£;ÙË@ßn"³*å?üכ'˜™?£Ú!þNò?§Ë
te@ždoa'@
v4‹¢àë¿ÊæW¸M¹Ç¿Ü{±|9av¿Úä1ò¿Üžt?¿Û#'K¯¿ãO"þ)f+AGNbll3FGL J0953.0-0839PMN J0953-0840?ïþÅ`ß$?±ëy
t?#¯úߌV?±ëy
t?ïõE†
àH?Tb9ñ"]•?Ut󚈁??Tb9ñ"]•?ïíç'ÁÌû?eUߧ=S?b}<Ó-W?eUߧ=S?ïõ—Gôz*??MŒ(Ñ«]?TÑoþN|Ë??MŒ(Ñ«]?ïüY€¶?8u–[Å;¸?=3ü+õÝ?8u–[Å;¸?ïÌp~½[?âq%égó?yÇó-c']?âq%égó?ï硈aŸ?r´K;U¦?h^w€$]™?r´K;U¦?ïæø(‹Q?Wùýn·–?i×Ö9^Ñ?Wùýn·–AGN4FGL J0953.4-7659¿Ô©+|xUÀ1Š©Å`ÇÁÀ:½c€ßÀ<`wç˜*.@ ø£8bG?þ¯(¬ÇsÇ?ÎÙh¼ûî?¡·×GO÷?Ñí_‹Íÿ?üY˜Ý±÷^?îz	{©ÄŠ¿æ³"µ!¿ãÞÞyÈn¿É@٘b7¿ãûD^Ô¡­¿ÇZ<!~|AGNbcu3FGL J0953.1-7657cRX J0953.1-7657?ïþU2-ñø?!—pÙE?*¬ÙbOâ?!—pÙE?ïñ†'2J?_;½'Æa?\òüG‹N?_;½'Æa?ïô¾®Ú|?Cm[¡å?V'¡Á—u¹?Cm[¡å?ïê¨åçÐß?H̦s‰	?eWЈæ?H̦s‰	?ïþݤœ"/?ÑDwþB?"%µðn¤t?ÑDwþB?ïÎuD‹ÜS?€¼bnÍ?xÅ]¡T¦±?€¼bnÍ?ï÷ÑÕ(§?b1sð†ž?P\U…f8M?b1sð†ž?ï ,·²Î
?rÍt'É'é?‡ôÒ!
ì·?rÍt'É'éAGN4FGL J0954.2+4913¿Û7€ÓW´@Hɛ^•·À:¸®.|NÀ<iU1Š¼‡@!¼'?ò"EW"%Å?Ë*D¢s?ÔÍ¿Ü#å@
)
]Qï?þ%2êc
¼¿ïêzAå}ž?ïý³^f¾¿ÙÊɝ}u?ÒóbÎ+qž¿ÛV¿\W¿ÐtéæAGNbll3FGL J0954.2+49131ES 0950+495?R;êš? ɦ(?\ëttõ_? ɦ(?îìDJÌq?­÷Ù#žõâ?¡?;»S8ó?­÷Ù#žõâ?îõª{£?•!­·? ¥XQ–CÐ?•!­·?ïaEæÐ?Y?€/àä¢ÿŽ?"×C'¯âÕ?€/àä¢ÿŽ?ï::òÖ]?–#æzx
6?˜¸¡£|'?–#æzx
6?êëªeGm?Ë6
ÑȽ§?ÄQVk¾âK?Ë6
ÑȽ§?ív²ˆ—­?§"6åßO?´ORjß[–?§"6åßO?í$ª#Z£?§fvÙ/™'?¶Ú¯ÏSg?§fvÙ/™'AGN4FGL J0954.2-2520¿ääMÕJõ@6_Až0PÀ:¢Iøq–EÀ<~ÑF¯ú@ /
Å"?ÿ‡šÉD'?ÄqÁ¹H`—?˜Žd.d?ØÁ—¯@÷
ú¯ß?ïÿ!ڛB¿Ür½'ÈF¿çp4摙ñ¿ÄP'à™³E¿áHÍcˁs¿ä'gÁZRÝAGNbcu2MASS J09541965-2519588?ïü›¢ïiì?-½©‡.Ex?;"ç—2o?-½©‡.Ex?ïñÕ:¸c?]»škjÍú?\UŠ$¡j?]»škjÍú?ïñ½ò`Òu?Q'=.ߑv?\"áö
?Q'=.ߑv?ïñÄz1¹$?=ˆ6"©?\wæÅFÉ?=ˆ6"©?ïü'‡1˜?8–÷2'f-?>ÃÅ·?8–÷2'f-?ïÐdx\?z­‰1_Ó?wÍøÔçO?z­‰1_Ó?ïò8ržiH?eÝyž'É?[Ök?=?eÝyž'É?ïÏ5×ʤ ?cî·¬tÕ¤?xeÌ?cî·¬tÕ¤AGN4FGL J0955.1+3551?ïüãŽbâV@Iß°_®¼AÀ; ˆÂ±ÀØÀ<ôæ¾æZ=@ œ"†Z"?þ$àŠó?ȦˆÂÔ?™µ÷ü®ðL?Ô|Š_iòã?ü¼xÁ²½?ïüÿ?:Óf?Òß<ã[/¿à¢»ìª¸¦¿à. ÿÿÕ
¿áÃ_eÁ$ù¿×m\D#›fAGNbll1RXS J095508.2+355054?ïý¢ŸŸ›?,3H¯Þœ?2ë\df¨?,3H¯Þœ?ïòþê?Y»ó¨Ý?[èƒvS?Y»ó¨Ý?ïä‰ã Ô¿?r*?kv»oPÊ?r*?ïÙ3¥p!?Si­ €o?sf-`ªGŽ?Si­ €o?ïü½ÓŠ¬?4ÌК‡?:b<|%—?4ÌК‡?ïËîŒÔÓñ?zٟ›t»Ã?z¹Õf?zٟ›t»Ã?ïԔ4ˆ{m?xÍlh?uµåÀ'½œ?xÍlh?ïd—‡'?}ÄjÍ
¸?"m©èRW?}ÄjÍ
¸AGN4FGL J0955.2+0835¿äÑÔX²H½@F=ã!¢ç÷À;Fiž)KSÀ<™§ågÎ@D‡Åܙ@ø¢×/ý?Õ@'&5t?³Ä»[`Mó?Û£VœCíì@4§®/RÔ¿ç=:¾Aê|+"Ù@y¿ç0iTWp)¿Ò¦^äfòR¿æuÌ}ɯ¿ïò›]¾÷øAGNbllNVSS J095501+083342?ïýÓI,ˆŽ?%tA]Yµx?1e¸»ý­y?%tA]Yµx?ïóGSŒÖ#?WY´…7÷»?YqXžÛÚ}?WY´…7÷»?ïñi5'wÖ?cÃ÷"e
Ï?]-•("m?cÃ÷"e
Ï?ïúp1ýdU?.zá']ΐ?F?8ú 5"?.zá']ΐ?ïþÓÝÀÄ?#b›æ?'âÃÌ]Ñ?#b›æ?ïÈ$óTv?"ÈlÛH~?{þí¦¢×?"ÈlÛH~?ïï±3RÃ?mSÄ4ç*)?`NÌöL$×?mSÄ4ç*)?ïÝ]š 8k?c80°n?qQ2Î犺?c80°nAGN4FGL J0956.0+3936?îÿÿƎ0@IÞ<âž4À:ñù²%hÀ<½>Õ'å@`ÕwuW@Ò7y…?Å
½]Äu?ªéLŠGA2?á…Ñqw<?ý"È<V?î™Ä%^¿Ö‹_ú¼t:¿èŸœb¡µÈ¿ãV:Ÿ8?¿áBUå墇¿ïÿú Âî'AGNfsrqWISE J095608.57+393515.8?ïûFÚ|Z;?67üQ!´?Bä—_˜ô?67üQ!´?ïí™K'/?b
¹à•?bf´Íü?b
¹à•?ïÔþ •r?yR‹Û›g¿?u€¯½pW?yR‹Û›g¿?ïÃ_£~ŸÃ?aÀ滑‹5?~P.#Óf"?aÀ滑‹5?ï÷[¸õ?G•°•Üc)?QIÈAõà?G•°•Üc)?輦"K.}?òåðr3ó?†Y÷zòÐÈ?òåðr3ó?ï¶Ð½ƒié?ƒ*AÒEM5?'KС?Ù?ƒ*AÒEM5?z†%k?'¼(&õ;?¥×øYUwO?'¼(&õ;AGN4FGL J0956.5-0958¿ï«.y5@@ÖÌ¢Ûa»À;‡þzÄÂ<À<¿Ã€ó°f@!ªpI¿Í?õ^x%«‹4?ÞH×à&?Ød¡ŸøXl?úª(Èv%÷@Æ+rõk¿ïúŒ"¸'¬?ïÙû¿(Ÿ[¿çã4å2t¿½‡âž+ŠÙ¿ÜNczΨD¿È§^hÁ	 AGNbll1RXS J095627.2-095720?ïý"§±#?.{/´;ž?7›ZUœàJ?.{/´;ž?ïò\…Uٕ?\÷²eQ+?[FõS
?\÷²eQ+?ïÊ;#±NÜ?yÊ=¦S¼@?zânš".?yÊ=¦S¼@?ï÷]æÔϔ??cÌ7Ôې?QD2V`×(??cÌ7Ôې?ïýä£P?-°p'à­?0ß
ídáó?-°p'à­?ïÍ+°°U?z(Ö©h›T?yj(DÝt?z(Ö©h›T?ïÛt´¡¡•?y#£1–¥œ?rE¥¢ ±½?y#£1–¥œ?ïÞã‹]Ê>?g¢'ø –µ?pŽ:`éÒ?g¢'ø –µAGN4FGL J0956.7+2516¿ÓÖцM•@IzÒ4ëšÀ9FÁ*ØßÀ<Fx*´±@zŸÉ3%@ç	#•0~?­PLž"*?¸cÐ^ý'f@~5Å´ª—@0ïŒv¿Ðû"‰µ ¿ä¤
ájÿçb)Àê¿èû¶ßû}º¿í¼{Eñ¿ïúàSG%AGNfsrq3FGL J0956.6+2515OK 290?ïýÊ1Ö«?!Üß{Ò?1®rŠ˜Òµ?!Üß{Ò?ïö(9É¿?Q"NÐÂUž?S¯Œ›<…?Q"NÐÂUž?ïç)Æwô?`1G?hÿÖ ÊÜ ?`1G?ïóítÀ¥?G+‡X»î?YÊ$¥Ë†õ?G+‡X»î?ïþI1!`"?bm¦ˆ›?+lê<ÏK–?bm¦ˆ›?ï׃KÆÊ?rH&>7ö?tt>y¹®?rH&>7ö?ïÞúöš•\?q|ŒYFm¥?p'"—è^5?q|ŒYFm¥?ïÐкÃ
?h©9'ýW?w—¢‡§ñ?h©9'ýWAGN4FGL J0957.3-1348?ïq¨ºÚî	@?.+{®ÍÀ9¦©ÑAåÀ<*ø; ‡@SŽºB†@zÕٻș?¶r ®Ì1?Ãà:±@0
ÚN•@úÓ>«âG¿Ëƒw™?¿á†"S¼ì¿äŽ4 C€¿èqéòwA¿í$ŒVºø¿ï髕D CAGNfsrq3FGL J0957.5-1351PMN J0957-1350?ïñM+›©?Zc†£©?]e¨'´;ê?Zc†£©?ïò¢Á­×6?[‰+<5¼®?Zº|gØu?[‰+<5¼®?ï¹×ߜÖ?{ºkðï¹Ý?¹ÉúZZ²?{ºkðï¹Ý?ïúØmd ?-·2öT¥?DŸ­‡E¯¼?-·2öT¥?ïë³>¨©¤?^'8"š'w?dLÁ7¹óá?^'8"š'w?ïÑw™ ½?XHXœ?wD3‡~%€?XHXœ?î¿Ú±šté?œaL ?µ?¤TéÈMe?œaL ?µ?ïìÙ%[ëI?Püº.?c&Ú·R†o?Püº.AGN4FGL J0957.6+5523?¬‡Yk¥AM@G÷7âÅ\–À7Ìo¯»DÀ;+Šƒ|!@º	^" ?þgbzH›z?ŠñnÝ`÷?´
š7Ï$@@%Áã†Lµ»@
%@톿±ªà=íÌL¿ØběOý¿à•OB2"¿à[
bY'l¿äS¡2OB¿åTWp)]ÇAGNfsrq3FGL J0957.6+55234C +55.17?í&Jãº5W?¾ÄRY-¸?¶Í¨àv‡M?¾ÄRY-¸?і™LË=^?ÆC7çfÅÌ?ç4³YšaQ?ÆC7çfÅÌ?ëýá¨1?¬CJé™ri?ÃÀxõ_=?¬CJé™ri?ÑߜT¬L?¸¯¼9Liõ?çr1Õ©Ú?¸¯¼9Liõ?ëâÄ'Y-?Àé ³e?Ðtïb›M?Àé ³e?°Ût
æ??²Ÿoä—ÙK?íäñ9‹?²Ÿoä—ÙK?íÖa³Ï$ì?¥}ñõàž9?±Lòaå"?¥}ñõàž9?‰?¿\‰?'uJbu+?ï›'Ž?'uJbu+MIXED4FGL J0957.8+3423¿ç»£…¼Ô@J&îcŠ	À:t¥×ÛÀ<®!õô
ƒ@)ÒÉ*@q<%J<d?À–%›Åî·?ĸØú¹>@(C(†@Ž e¨"?ïû›¢|K¿ÜqÎäÕO¿ábTŽ†@¿âWÝ6§[ú¿ç¾RúÉ¿ïöCôK–×AGNbcuB2 0954+34?ïùÉÆÌÚ?FËî;øRŽ?HØçXå4X?FËî;øRŽ?ïôVo‰‹ì?Uíœ~8¾?WS Ëëèÿ?Uíœ~8¾?ïáßðIv?i™óp¢lã?n êýؒ?i™óp¢lã?ïäox³Åë?M81­
á?k‡:\h?M81­
á?ïóÒ®ŸKp?SXFƒl?XZ£JÙ~G?SXFƒl?ïÍø¶h:?‡À¯µLs?y~ƒ·YÆä?‡À¯µLs?ï›/f¨‰)?…øÝÀȯ?‰4&KŽá¿?…øÝÀȯ?ï¨Ä—ŸŠ?lÞ­q&+¸?…ÎÚÊA¡?lÞ­q&+¸AGN4FGL J0958.0+4728?íþÉLmI@IU·|¯ÞÀ9›"²ÈÀ<1Ø2[@¿B4Íg@ì&ÿ½?²SõuuÊ?Ð?½t•@ge47?1@ùnõG¤?Ìÿ‡	I)ë¿Þ²…³¹€¿éTÀ¡›EÁ¿ç‡»JÄIq¿îíŒàΌk¿ïÿ "_õAGNfsrq3FGL J0957.4+4728OK 492?ïTé å_¸?Ž7û ÖC?•bËëëñ?Ž7û ÖC?ïôÓ/×!ÿ?V=MI|#Q?VY %Á?V=MI|#Q?îîæä6\?šÝSŸè§Å?¨"PO;?šÝSŸè§Å?ï÷BOÁða?=»ÀpKLg?Q{`áÓ­Y?=»ÀpKLg?ïA'·?•*TA"­ž?œ?—ÔúA?•*TA"­ž?ïÎë‰ë¥?zsOÞZ­ç?xŠ;'E?zsOÞZ­ç?íH99Ýq`?¤[ò¾X?µ¾62ÌC?¤[ò¾X?ïØèø¸Ÿ*?bŒÔA9Ì?s‹ƒ…sÛd?bŒÔA9ÌAGN4FGL J0958.0-0319¿ïOÛÎ%@C%? §?À;œ¥ŸaY·À<Ê]Óð­}@"˜ÕV‰#«?à•<<Ç0¬?ï6jXŠÜ?é±e¾àÆ?üõÅêZ|@²Òû¿ïýcm¢?eÆ-¿ÖUGZ1¥¿í€ãŸø†?ê·ãÑ̿⨈ŸÌ8¨AGNbll3FGL J0958.3-03181RXS J095806.4-031729?ï/N¥æ•1?¿Ë®û¼¶?š+?½½ã?¿Ë®û¼¶?ïõam¥—K?UB÷øZ~?U=$ŽUÉÛ?UB÷øZ~?îÕ_èóÉç?—ÄɎ¢ò=?¢ªn/¬˜?—ÄɎ¢ò=?ïþÁY2?#S±€ñ1¹?#ïÿ™Ñ"Ô?#S±€ñ1¹?ïÚû­¦?•" 辪?ró'-–5?•" 辪?ïÓ$ª\?w£2F'›\?v|m—
ÊW?w£2F'›\?îp'܈y?œï-ëbɀ?¨öÒ7xoÜ?œï-ëbɀ?ïü÷E'|X?B©wœÂ~?8EÒtÐS?B©wœÂ~AGN4FGL J0958.0+3222?ëyYnl€@J!æî·`À:oÎ=UÀ<A©î{s@{k™¬@Ý«ýIl[?¼u_þmXÉ?°ç1ýÔÉ?ðmjœV|@"ëa¸W?í™j4Q@d¿ç@6¡|¼ê¿çE\á,€<¿æLs@i|›¿ë—¬ÂkJ¿ïõ´¢‰'JAGNfsrq3C 232?ïñÐÓJH?WÁp…÷?\^Y²çÞø?WÁp…÷?ïìšÙ›Îc?bZb+?ce&D•4Ë?bZb+?ïË)Y{Ç?wP~1)t?zk~\1N?wP~1)t?龍ð®î?o'c
·?†ÃÛ#·?o'c
·?ïͦo¢±?rlê0'KA?y,ȃŸ?rlê0'KA?ï³zðùÂ?"ÞŒS:-±?ƒ!~SÃ†?"ÞŒS:-±?ïÀ²âJÎ?€©ŒŸÃѽ?¦ŽÐ·ðÌ?€©ŒŸÃѽ?íýÞGÇ?š+V7G©ˆ?°4wí'?š+V7G©ˆAGN4FGL J0958.1-6753?ЅîvÀ¦¤À$™ë…¸RÀ:ö•mºîÀ<C¾˜V£{@始ʣþ@ùPá™ãk?¿Yô›¿´B¾$=w?÷­N·ó÷´@Y±rµÕ?Ԓ{'­Cð¿ä¿ð{'¾‹¿èH4rß¿áŸÿ¿"SY¿å´ÊAؤ?œñ(™À'AGNbcu3FGL J0958.4-67521RXS J095812.8-675241?ïýõì"Iù? «"*U7/?0PŸ'öb~? «"*U7/?ïïב ú!?eÅJÓv?`(nòC¯M?eÅJÓv?ï÷œî|Ž¶?]_T¶%†?PÆ#áT?]_T¶%†?ïù(÷VIt?6Œgèn?K\#§	ۇ?6Œgèn?ïüÛP{Ì?5£ìÕêüb?9%{²'Ð?5£ìÕêüb?ïƆ}™D?€@¤|ø+?|¼Á<üÚ¹?€@¤|ø+?ïö;±µ?l³)èM³?SÊ;REƒ?l³)èM³?ï¶Îñó«f?tþÄlZ4?'LCˆ"†Y?tþÄlZ4AGN4FGL J0958.3-2656¿à˜›± @5Éó×ӑÀ;EeÄ÷1À<ª%s@-ÑRB˜?ÿùI²Ñy?Óû¥ˆ€?ÎrW`dÙ?üX(&·@õ^'?¦ÏF_ñéM¿Æƒ¨9¶°¿ÑߥA˜{·¿ßƒÄKžå¿æ8ßå®E"¿ïý²èõø?AGNrdgNGC 3078?ïð1‡Gß?WÎ0­ýi?_œñîê`á?WÎ0­ýi?ïÖ-'oI~?xѕäP0?télc(4ý?xѕäP0?ïϳÊnK?rQ×^Z?x&äºV·?rQ×^Z?ï´Ú' ?À?^و,>äK?'É[žwR?^و,>äK?ïîr4-Œ´?`:¤?aËÊ4<V?`:¤?ïajÑZ%:?›î'Ø$é?"Ò¥ÍÜ »?›î'Ø$é?ï]ë·.ç?1)D|C¹?"B‰"º%f?1)D|C¹?îpê$M¬?Žñc'ÉI?¨ñ^ró>?Žñc'ÉIAGN4FGL J0958.4+5042¿Ë_ËñÊL@HâãK"SÀ:bŸ1‰À<²Š¬–Ì`@iÂp}k'@ûµ¤at?¾ª ¹.Æ?­s\f³=?ê×'[å@
ڧ옚?â<x¡|g¿äÿïÕ¿ço˜p"¿èàíìEz¿ëèߥ¥¿ðAGNfsrq7C 0955+5054?ïý	戵œ?+5¬{pÔ?7°Êw}ì?+5¬{pÔ?ï÷ÑÄ>š?P'ñÄÎZ§?QÎ\ÉùkŽ?P'ñÄÎZ§?ïêdo7½©?e±,ñÌs?e›œGWX?e±,ñÌs?ïò̹xÿ?F‰4î?[æf	è?F‰4î?ïüž‰m|…?2ûÆ-´U?;¶zÆÛ?2ûÆ-´U?ïÛ^«ºŒ?q™ŒU{Ä?rPª!Z"u?q™ŒU{Ä?ïñL"ƒ/?csãäÎo?]çfúµ';?csãäÎo?ïȉ3ù_[?hÒ 7vÆ|?{»e×?hÒ 7vÆ|AGN4FGL J0958.4-2441¿êè
yfÚf@7|#̍ãÀ:rçy }NÀ<WË/=Û-@º+Kˆ?@	`Z³«?Áw÷ˆàd?É øžï"@È9À.e@)Ï/þuf?ÓÏ6JÀ¿ÛQc'A¸¿ÞÓA:ÝÌy¿âQ(Fp&Ú¿çñðÃL¿ðAGNbcu3FGL J0958.6-2447TXS 0956-244?ï£ý~NC?"3ªØ€g?‡ sYgE?"3ªØ€g?ïÔ âte?u¢)+æ—]?u¯Ž© ª´?u¢)+æ—]?ï¹%'¾L?}¿Êša ?¶›¾¨ù?}¿Êša ?ï®Ì8Ó0>?]¹á=•2g?"LñÒÃh?]¹á=•2g?ï'r]ën?™D»w¹?œm±µú`I?™D»w¹?ï,ºÍé#è?¡OƖñ¬R?šh¦Bۃ?¡OƖñ¬R?í'ž¾WÐ2?¨¤¢d™?¶Ã
e—s?¨¤¢d™?î)œ³ýQ?ŒBÔ+‰ó>?­f7è/Æð?ŒBÔ+‰ó>AGN4FGL J0958.7+6534?ÕAlÓ#9Q@EYtæ[êÀ8rÐ4³À;´~d‰íT@êƒ-±@Kv Í|?"åL"C>?¢ÿPËN@BåۑŒ@¦±['1É¿·(ÃÂ>~¿àåÜhKBô¿ãƒÿiKZ¿âýò^¬³¨¿æz¿^z3οᘼúDZÛAGNBLL3FGL J0958.6+6534S4 0954+65?ïþ-…§ÒË?!@È·…?-'¢'Ânš?!@È·…?ïøVÄ:Šž?PÎÓþ¶Ÿ?N¤ðEƒR?PÎÓþ¶Ÿ?ïé>§§ñ™?p¾`äùi»?fÁXl¬c?p¾`äùi»?ïÿîBt!>Ùï?.Áæ°>á¾4àG=>Ùï?.Áæ°?ïþlà†›™?"ð,"¹%?)1÷†áÏ?"ð,"¹%?ïÞ Z2?qÓßI&é'?pïÒÔ*f"?qÓßI&é'?ïÝlm͟?w"Ð[?öI?qIÉr?w"Ð[?öI?ïÿóvH>Þ[9y–
>Ù7éÆ@>Þ[9y–
AGN4FGL J0958.8+7039¿×ÄC¹	ÃÆ@D$ p¹À;Çp‹ÔÀ=%Æc&@@!í³/³ø?øÿ&¡Txþ?×ÚQðœ5?Ñ${tëdh?÷ ªêúµ=@ߘ¬^ÿѪN½Ó4Æ?Ö{4©«?áÝhã³?³àΌj‡¿çP䉁ôa¿Ì.îúâ	AGNbcuGB6 J0958+7039?ïúãðø©?6'oRc<m?Dp<ѐÚ?6'oRc<m?ïòe^å¥?[ˆþZP:û?[á51¶–‹?[ˆþZP:û?ï׎–Ӎþ?puUtØ?t8´'û0Ü?puUtØ?ïÀŸi++—?eø¾4%?°KvÈ̟?eø¾4%?ïù³'_??C:0Ū?I3ax`Nø?C:0Ū?ïΦÓá5‡?x´Àñµ*?x¬–èy?x´Àñµ*?ïÏ :-ßr?|þ0	A¤?x/âãæÉ?|þ0	A¤?ïlÈ|tßj?ƒIð'߆Ó?'fðo¬DÉ?ƒIð'߆ÓAGN4FGL J0959.4+2120¿Ô`¶ y¯@IH8Ÿƒ¾fÀ:§]u&ÊÀ<…='[·@€Ù% £y@"NCYñä?Àªa½à濋—/Üçw?Éü»§áZù@gNåúÆ¿ˆ@ïÎs¿ßpš1o
Õ¿áéžÊ[…¿ãgS–€	¦¿ß†3‹GÇ?¿á¹ASAGNbll3FGL J0959.7+2124RX J0959.4+2123?ïùÛ$Üâ?x;"–JUI?Kü"Å›ñð?x;"–JUI?ï÷xi8u?O—IÄuÇ?Qùõ¯?O—IÄuÇ?ïôœŸˆpý?^•r,íÌ?VÆÁ#X1?^•r,íÌ?ïú/½C(/?.Fæ­¨é®?GA¨=æ'?.Fæ­¨é®?ï÷:H/§?IÍ'¿*5Z?Q‹o‡éÃ$?IÍ'¿*5Z?ïØ%"¤DÃ?xÈѦ_‰?sín›ÿ¦o?xÈѦ_‰?ï뤟˜Gp?qHÊðæÉÙ?d[`m7ï»?qHÊðæÉÙ?ïèÜ?†}³?T¿œ'î
?g#ÀTf…*?T¿œ'î
AGN4FGL J0959.6+4606¿æ­VBŠr@I¤¹#¢œxÀ:¾=¢ø½ìÀ<u¾{Ñ1¶@$›7(‹:@Róš–ï›?Â×ø…bU¿¤E_@éep?ÚµgÀÙyƒ@=Ò™™?Ú/é(M&¿á­ïýS}V¿ê^ç$.³¿èP"Xð\¿ïÿòÿf}
?ïr·bWcAGNbcu2MASX J09591976+4603515?ïø«ç
Kï?QñE¼¾ˆ?MPd› G^?QñE¼¾ˆ?ï´×
?b²÷Ñï´¡?ajc.L;f?b²÷Ñï´¡?ïœ	Z–?ª£üÐ?ˆýœÊçÊs?ª£üÐ?ïÜ­®6Š?]NxÔ²´?q©q²ƒ£?]NxÔ²´?ïâšýôþ?s<¾ïR×?meÙAö?s<¾ïR×?ïs#—΂?—uÁœCÍG?'›ŒÿP"\?—uÁœCÍG?$È-Î?ˆ	Ìa¶áû?‹öÑd(w?ˆ	Ìa¶áû?î\›6|¿?Ÿò¬#l¾0?®š6Jàf?Ÿò¬#l¾0AGN4FGL J1001.1+2911?›ËjՔz)@JOKrÅzÀ9z¿ª¥Z˜À<^×,¢z@wÐ1[AÅ@ä#¾K)Ê?«ÉªƒvÂ?®éO[Õ5I?þ¬5}N—@kd°-Û?ÁZê‡GÝd¿áÜ,¼ ­¿ä¾ýÝ;¿äÍi_•ô¿ã˜†t"è¿ß¹ö{œÙjAGNbll3FGL J1001.0+2913GB6 J1001+2911?ïþý寭é?KÁAä &? !£¹úi?KÁAä &?ï÷Ÿˆ¾Ly?PpŐÀ?PÀî§"þ7?PpŐÀ?ï÷a·fDi?;ž,ԝ[?Q<'›ëM×?;ž,ԝ[?ïÿ}d7j®>ÿõ†*mz?Su\)Ú>ÿõ†*mz?ïÿ ý%°?&Â.du?àS
í°y?&Â.du?ïÜÆoïâ?riV;é½?qœÇö $?riV;é½?ïöJX­"ø?YU±jJ?SkNÅòP]?YU±jJ?ïÿ,‡Œ?®?¨iÝy™?o
./Ëò?¨iÝy™AGN4FGL J1002.5+2215¿ïwð7¸ö@IÂ/¾3¬ÖÀ:Œ¬nˆs×À<wXï…^y@ žv{‡_Û?ýä(3$ðz?Å‹ypYY?›˜+§Åù–?،üÓ$Õ¢?ðÆ+«T'
¿Úם‡ý¿è
ÀGƒLP¿ä.]
¿Ô"ãQs¿áƒ÷ÜEÕ¿ÕÝÖÿžAGNbll3FGL J1002.3+22201RXS J100235.8+221609?ïûÂÞâN?9Šš<dt?@ôƒ–Ç?9Šš<dt?ïà
2‡UŽ?rmi	5ã,?oòÍDpb3?rmi	5ã,?ïèë>z±?gÇ!7â
?gú€ì¦ë?gÇ!7â
?ïÉ`~u?qԞŽ‡(?‹Í§à{¢°?qԞŽ‡(?ï÷üÌÕö?P®;TþS¿?PßéBLù?P®;TþS¿?ïY€à™? M†%°?"ß~õVâ? M†%°?ïãkñÚg.?wefxèC«?l"
é²Y?wefxèC«?íoü#žâü? 1óp/?´€äRž? 1óp/AGN4FGL J1002.8+2140¿Ûï›¥Ã@I³ÌcñA À;c$W@YÀ<ÂWþė@ÖZÖæ+C@˜ûyˆ'?ÊôµÉû⿦³vºq€v?Ùy3]$žE@‹ž†é=ǿ什ÿT‰o?îE¶Ãvö¿é=1ïfTÉ¿ÒUUM9¿ïªøÎÞ?åo‡wX&2AGNbcuNVSS J100250+214225?ïÅݬóS?´<ºÅ÷3?})æˆÖ˜?´<ºÅ÷3?ïöa§Ic?SO#±çjq?S=Ï`¹?SO#±çjq?ï°.ÝtK?€ÀK*éí(?ƒôH­"…?€ÀK*éí(?ïú8w"‹?4½¦RvË?G߇îê?4½¦RvË?ïëºÃz¿?jfÇô|?dEåK1»?jfÇô|?ïÍïj97b?öëS%?yJüÑjø?öëS%?ï™Àú)&?‰Dâæ6?‰Ü4&R?‰Dâæ6?ïÐVå
?pTZgx_?wÔøhÿ—S?pTZgx_AGN4FGL J1003.4+0205?Õâhm°:N@ESøüÖÔÀ;9|"NÀ<¬#þ	ù@Óy³J?ÿpŽ•·?È´ E°8m?°Ü_çÇ$?å•ò`L–?ÿµ³–??ïî"%âؿꐀýÁ?³$œ—zÛh¿è¢JBCqo¿Ú¹#ã	$A¿‡.tɉ)AGNbcuSDSS J100326.63+020455.6?ïý«6'O?(íˆBÃ[:?2¦MÜßuÃ?(íˆBÃ[:?ïðÜí3þ?`å8€.v|?^F%yÇLF?`å8€.v|?ïê˜{ìq?aÜ$pZ*£?egývUV?aÜ$pZ*£?ïêœÀYe¼?K§Õ¼>¾/?ec?ž[4V?K§Õ¼>¾/?ïý1CmX?,iCùydã?6uç컳K?,iCùydã?ïÉ©^UV?{¼Ã2ûÆ?{+PÆV
?{¼Ã2ûÆ?ïèë~"®É?o¨iþÕ-?gaRw?o¨iþÕ-?ï©Èó›ºþ?t—
êû"<?…Ã2p?t—
êû"<AGN4FGL J1003.6-2137?Ð-4‡Ï @:ÐEþÀ;ŒŽ·¾HÀ<À
(ÝnÛ@"ÿ2ûé?ùú5 Ë½?Õ¦_»&‡(?ÀJ
MzÝ?ëbC¡ÀY¢@#fón¢¿éaßî聿é/"þ)f+?ï:Î2'šy¿Ø7±G5H·¿Ø5H Öj¿×A¼ã˖íAGNbcu1RXS J100342.0-213752?ïÿ\;À•?š»Éï"?xH?š»Éï"?ïôp"©£?\–8X?WÙõ(Zm?\–8X?ïøÌTp´?<%ïªGáì?O°ÎwCnÅ?<%ïªGáì?ïû»Z3¨#?/Ÿj	W 9?A–ܵàÅ?/Ÿj	W 9?ïÿ_ï¯ó?
¡&¹(Þ?ü>‹'é?
¡&¹(Þ?ïԀ¡aJY?x?àéÚç§?u¿¯\iWp?x?àéÚç§?ïú"Àā?OI–š^W#?G'î'N'?OI–š^W#?ïöÌ`Òc÷?IeZª|¼Û?Rg>#
?IeZª|¼ÛAGN4FGL J1003.6+2605¿ìMdø'C'@JTX`fÀ:›k¯{ƒ.À<wú ø@
?h ¨W@"¿'a?Äð!e«U"?Â3£Æn8î?÷O­¢e6?þš<â(¿ë{L§xn¿Ù2ñ#Ä*g¿ãrZ?çvœ¿ç[§J¿àÑ۔æ¬r¿ïüfM;òõAGNbll3FGL J1003.6+2608PKS 1000+26?ïù RÎâ"?A™÷4[>?I~´ÐŽ(V?A™÷4[>?ïäfÒ¥‡l?mg‡¹øRÅ?k™-8|
?mg‡¹øRÅ?ïÛ0	í?dÌf‰mšÂ?rgý'z	0?dÌf‰mšÂ?ï®þ2þã~?joµíÿ¡²?"@s8?joµíÿ¡²?ïÑñ¦dÇð?q=,ïê:?w,Þ(&?q=,ïê:?ïaU³Ê{?–PrA¦?"ÕMî®›?–PrA¦?ï€á<y
¶?"z°µ5?Ç°èœŠZ?"z°µ5?íšWLB"å? Œí¾Óȑ?³-EŸ¦¶Ô? Œí¾ÓȑAGN4FGL J1006.5+6440¿¨Á°õ6ë}@F&¯%;À;*.XØß*À<ç3cښì@ ÷êÃز^@©}'Ô?ºrzù*¤¿¿Õ€r'?òXåªda?ÿã­¹â}¿íÐQò;_¿á½c£=‡¿â\ᢜ́¿ÖGKCdt¿ä	Úÿë]1¿²zs8±ÍBAGNbllRX J1006.1+6440?ïý2ØfÖE?,,E}÷P.?6i<H©C?,,E}÷P.?ïò3Xioþ?Wñ"Vb¥û?[™O'VTs?Wñ"Vb¥û?ïòò¹"T?Rãp°Õ?Zë՗r?Rãp°Õ?ïåÕ9> ?SŠ"Éjý?jâ*ô·d?SŠ"Éjý?ïù‹¼â?BTã¹pð=?IÑù£?BTã¹pð=?ïć%V?m¿Mî­k?}ñzSʬ³?m¿Mî­k?ïïÞá2›š?mVʆ[WI?`!¾F5?mVʆ[WI?ï[KˆÈ?Œ''c?œ´–‹w`í?Œ''cAGN4FGL J1006.7-2159¿â›6®¬•@:Æm½r¼¶À8aKŸŠÀ;ÊÊ·H×	@ê'1È$@ZaÎQ1?±!ð@+?§Œ%'¶¦p@хÞz@¿´Û>˜¿ÂŠºX«è§¿â}Wyc™-¿æ8"œ×%¿äÙ>ö
¿äìÉA|÷ø¿èw]š
_AGNfsrq3FGL J1006.7-2159PKS 1004-217?ïþÛè?17šõ$v?"A}Ej®p?17šõ$v?ïõÚgŸ=?Wãd…¼ö?TK1à'v9?Wãd…¼ö?ïðj9•ß?fñÒW0¬†?_+9öY+?fñÒW0¬†?ïÿ÷.u3^>É_£ØÄI>Ñ£Œ4­/B>É_£ØÄI?ïÿ¬J¡9?E¶qÇùq?êpÇQ6S?E¶qÇùq?ïÓæ?J¨?{d1"¤Õ?vàu
˜?{d1"¤Õ?ïàrfNér?q`Kõ@ó?o™á1ž?q`Kõ@ó?ïÿ÷;á,«>Ð8L0҄ð>шsWÊv>Ð8L0҄ðAGN4FGL J1007.0+3455?£Ïò;Q½@Kà?pÀ:š¯_Ô{îÀ<Š®¬Ÿ0@ oè;=B×?úùcc|§?Ã#öiÔ/?Á*¢jùs@Òz{Ç!@g&q÷?ïÕřҤ}¿â†ôæÇIÖ¿ËåÛf˜Z¿Ôñ§ãxu¿à ÇuË¿ÞE`Ý:ƒAGNbll3FGL J1006.7+3453EXO 1004.0+3509?ïü×jt?/î"`Ìä?9G£Ä¹3?/î"`Ìä?ïï<BÖ·?\efÑæ%/?`ý,`Ì?\efÑæ%/?ïó´‰Vª?Q-r}˜«Œ?X–î
Üt?Q-r}˜«Œ?ï¶ï¯"œt?`›Ï,b.?'D¡µ)?`›Ï,b.?ïñ:Ný¶q?SbëôŽ"y?]‹br†M?SbëôŽ"y?ï¹MSl[?ÇÖWŠâd?¬«1V4?ÇÖWŠâd?ïîˆ,p´?iÀIeµu?awÓ|»{º?iÀIeµu?ïIŒÙ(?"4
°'?ŸößÎdÚÿ?"4
°'AGN4FGL J1007.6-3332¿å
"4Ïã@1õßeUÅÀ92 
¼À;ûN']Šö@¶‹¤ô@<ï>çœ\?­ý"ÀÁќ?Éü§ZøI'@ÿõbLM@÷Æ0{s?Юý®ìè¿ÞÁ {öpŠ¿ær¡Þ¹¿èkˆVÚØ¿éÄP'èË0¿ïÿÀtϵµAGNfsrq3FGL J1007.4-3334PKS 1005-333?ï™ñfÆCØ?'è:–É|?‰ƒ¦QÞ¦?'è:–É|?ïÜ̉'}ë?}BÓbˆÎU?q™»{_R'?}BÓbˆÎU?î€ü?^Ã8?›Ý4™§ÀÖ?§ð<_O'?›Ý4™§ÀÖ?ïù3-²s?8²ó"é³f?Kã3ø•t´?8²ó"é³f?ï'd°?œ–l…½®?QÆ;ü?œ–l…½®?ïBÂR¨÷ä?§GB‡)£"?—§µ±À;v?§GB‡)£"?ì£Vrc°æ?¨ˆ–ŠB$?ºåLlâxÓ?¨ˆ–ŠB$?ïÜg#û‡Ë?`v±²G?qÌm÷=Zr?`v±²GAGN4FGL J1008.0+0620?ß,˜ú¸B|@G×süÀ9*¼ª?ÚÀ<¼ bv@Ù'ÌLÊ3@B+{®Í?«0ªþ×ó?¨)Ûúë?ü´d¬R@ºË…$?ïþ[à¦sr¿ÎBßN"¿ãíÔï°ýc¿ãˆ¿V"¿àºÇ犾5¿èZ€êv+AGNbll3FGL J1007.9+0621MG1 J100800+0621?ïþ•Î¢©§?¼¡ùL‰¹?&£‹‹
¡?¼¡ùL‰¹?ïõìQˆ™þ?Vᳺm'?T']Ss?Vᳺm'?ïð†ÑH?S¬mê
ÚD?^ò]õz¶?S¬mê
ÚD?ïû­Á!{ƒ?/Ί›³§ó?AHü{çÔG?/Ί›³§ó?ïþlÆ8]?!ßѼâ?)3 W"ÁK?!ßѼâ?ïÑ΋¶#Š?ygÉ-×ê?wºBzÞ¡?ygÉ-×ê?ïå¡á+B?s#)bv´?j^â-óƒ?s#)bv´?ïø]¯î?B|MÐÝé¦?OþŠUc?B|MÐÝé¦AGN4FGL J1008.0+0028?¹L	Cbº¼@EO'j@À:O{ûùáÀ<n,·/¢@1¡&@&býüÁ?Ì-µÅÊ$?»¢""EA©?÷'!A™'"@Y ­ ?ïÿü¥¬¨¿à"ßq?¿â&±$ÿà4ÚÓÍ%¿êø×ý­j\¿ïÿ‰XAGNbcu3FGL J1007.8+0026PKS 1005+007?ïïσ‹eN?UëkúmN?`0|¹Rá=?UëkúmN?ïê=[³¸‡?d~öÜéñ
?e¤Jç ´?d~öÜéñ
?ﶷˆS1g?6É#J¶ö?'RùùøG?6É#J¶ö?IðÜC?lÍö.ü/ü?ˆZí€YSD?lÍö.ü/ü?ïÜI| ºu?lT¿0ë"?qÛAá?lT¿0ë"?ﲏËÔC(?•|ŽÈŽC?ƒ\
§?•|ŽÈŽC?ï)H'®g(?"ŽÂ%)[?šÖû{Ló?"ŽÂ%)[?Wf]?Œl""°-?¦¥z…N«V?Œl""°-AGN4FGL J1008.1+4706?ïÁœ}¿ì@J4ÿëJwÀ<	zP(6€À=!iθ@"tRBÂó/?ÕÑȽ/v?ãj@ºˆ'?ï
{é…j@1¤Òh@|<yX¦?ît#=qÐ}¿ïÿúÁҝÇ?ïÿÒ†ëA¿Ü9™aܔ?Çaû'©¿é- qäAGNbllRX J1008.1+4705?ïù4֐3Ù?KҜòÍé?K,¦z¨Œ?KҜòÍé?ï÷ €S!?Q°x×ÏÙ ?Q¾ÿˆw"?Q°x×ÏÙ ?ïmÂæ«+?Œóÿ¼Ë?']‡£*š'?Œóÿ¼Ë?ïõ2£uæ?Jñ͖Úû?U›Øϳ?Jñ͖Úû?ïñ)½µúñ?cO¦òú´>?]¬"Ëނ?cO¦òú´>?ïÚðÕ¦ÌC?suªO ?r‡•¬"v?suªO ?ï‡XÖI¼ü?_­ó?h¦?Ž)Ê_ÒQ?_­ó?h¦?ïù"›ðè?P¢PEì_?Ku"ò_íG?P¢PEì_AGN4FGL J1008.7-2909?Ð:3¾°@5ŽÊW§†ÂÀ:Œ½½eP½À<ZTtÌZ·@qgd"(@ic¦˜…?È
£‡"S?̦C̪ï@€†
 z@
Wr,Ã,?ïÿÄ}îB¿å«fJ¸¿æ'F–½FG¿ä‡`F'´É¿ïý.>Åè¿îŠøìæGÈAGNbcu3FGL J1008.9-2910PMN J1008-2912?ïïÃ(օU?WÁ¤q2?`<×ós?WÁ¤q2?ïä¬SÞ?m³
§ìQ?kSã£D:‡?m³
§ìQ?ï¼2 ¶É?wM
}½*?€óxësµë?wM
}½*?ïÍíw?Z鸶Úc	?y	w#€>P?Z鸶Úc	?ïðRX<'?\Þ®mÊá?_[O	Ù?\Þ®mÊá?ï•Á·‰³a?ò/Œÿe"?Š'!Ã¥?ò/Œÿe"?ï•ZÖÌf?"/›#1ˆ?œMTŸÿ	A?"/›#1ˆ?îÎHç"=(?ˆB
ÆŸ?£qŠ+Éz?ˆB
ÆŸAGN4FGL J1008.8-3139¿ï"ÿ	F6@3˜>BZîcÀ:ç6žËÀ<•ohm¨@.tûª…Ð@^ܙÉjB?¹ÝâHßí¼?¦/³Ýù¬?íF¤>¹#M@Tóe轿âÖ÷ÞshX¿ä>Sü×W¿ã/c?•l8¿åú,hJl¿àlk΅3±¿êº¯"ÖáúAGNbll3FGL J1009.0-3137PKS 1006-313?ïú?ýŒ?XÇ?*_?E‹Òÿ»¤?XÇ?*_?ïïrœ³2%?`™zŸ·J™?`c)ë"?`™zŸ·J™?ïð-%ÁÊT?d÷vzJë×?_¥´ÔaWe?d÷vzJë×?ïò(žÒ
?A±ðU·)ü?ZᮺÛÖ?A±ðU·)ü?ïîåFHí7?VÉFVºÅŽ?a¹¹Òx£?VÉFVºÅŽ?ï¸Ìâh·Ç?"u%bç^$?ÌÇYsv^?"u%bç^$?ïÕÖ¾4¥ñ?{ïä%šHŠ?u àݓU?{ïä%šHŠ?ï±µÐíÿß?s
mmkS?ƒ'‹Ð.´O?s
mmkSAGN4FGL J1010.2-3119¿ï²	Š‡@4äy'¼À9"pæòèÀÀ;úio/bÄ@!PC÷¦•+?ûã#·;k?²'rásøË?'ÒóYçl?â3òí†+@
!"}ö¥ä?ÁrI«7?²L'S$¿åŠÛá<ÆZ¿®æ¤ o¿ä¦],+6¿Àf‹û r;AGNbll3FGL J1010.2-31201RXS J101015.9-311909?ïþâ´GE?ÜŠÒT?!Þ£~âæº?ÜŠÒT?ïòÅ9'
}?\ð§NaW¡?Zuãee?\ð§NaW¡?ïõU´‰×Q?]Èvº3À?UT–µWó?]Èvº3À?ïü•ògˆr?*¶³z?;PkÜÖ²å?*¶³z?ïþi…ˆHA?Þ;êe˜?)g©<¹?Þ;êe˜?ïÊ#A΁ƒ? °ôÿ?zî_ÞƔ? °ôÿ?ïô3ýn¼\?ftÝ:'?W˜·Sw¤?ftÝ:'?ïú"6©	y?<̏؇î7?E³$ó›?<̏؇î7AGN4FGL J1010.8-0158¿³ú'^žÙ»@DÍæÿ}úÀ:$<ù…'À<UäíU@q"–ØÊ@gÅá÷?»ÌBŽDü´?§M༠ŠÃ?è®~F¬ã@	–­…èÝ?îþê÷Z?¿æxK5ˆx	¿æ'bO*‹¿ãqYßofÀ¿ïýé:ø$¿ï4v"±ÓLAGNfsrq3FGL J1010.8-0158PKS 1008-01?ïü
Û=†?5y¹[B—«??@ې?5y¹[B—«?ïóH£¡Ÿ?Zý°íª€?Yn¹2ôn†?Zý°íª€?ïìü€w<U?Q‹ŸG»ÐÛ?cš¡¢Ä?Q‹ŸG»ÐÛ?ïéAûÜÁ?Sš^ö8‹¢?f¾ð+þ¶×?Sš^ö8‹¢?ïú™ Ðp?B±`"g?Gř÷V·V?B±`"g?ïÏW?›»!?}>n¤?xT`%ë±?}>n¤?ïîÉ-IÓø?iÕHRÉ`e?a6Òò¥'X?iÕHRÉ`e?ïµc>"º?päUž"Û?'º§,"¤?päUž"ÛAGN4FGL J1011.3-0427?âôî´©Œ@D
êÈ`V'À;R%fÁÖÀ<y_×Öì
@£òž­œ@Òÿ#a.?Õ&¯aû?ÓFÚÕùò?ü¶¡|¼ê@
™«Ã<Ö¿×w؞è
¿å9£ûkq¿æ€Éë£R¿åo쌅´à¿ïýÕ{Zi¿éÏ
í6ÐAGNfsrqPKS B1008-041?ïù_«ó?BRêBße?JRßK®˜?BRêBße?ïó›K܈"?Xÿºp¸Õ?XÉh;ð?Xÿºp¸Õ?ï·õ»¿šp?smL©çȎ?''
B
î?smL©çȎ?ïõ‹Uù?=QL³	ý?UãÏ\ÆíÌ?=QL³	ý?ïýÜ ¸é?.äþ%[±?1FP,p?.äþ%[±?ïÃSˆÊ?"Ø)Ý°?~V~(²KK?"Ø)Ý°?ï«4Y¬wJ?'Þ»`+?…2éŽõn?'Þ»`+?ï»ÔL™ó?nñ"GœT?
ûg-X?nñ"GœTAGN4FGL J1011.6+3600?íL*R¹á8@KŠ($xÀ;%t…
À<Ú\ђ.k@)©m¢ñ@"õÞ>Y?Ë|¢¨a­?ÍwY}ʱ@A@š$?÷KêlQ¸¿ßC\¡¹Ñ?ïȯÑêBÿ¿ßG.<ÔF¿¿ç™mYŸ®‡¿áó:u¿ïþ®üØ-SAGNbllNVSS J101147+360019?ïìu7ÿ9 ?bM†Γ?cŠÇè	/Ô?bM†Γ?îI‹9¯y?®kç®X ?«o‡NÖk?®kç®X ?ï…7Ê+x?"Ð1 ›p?Ž²
j?"Ð1 ›p?î6}ëhC?'UÍ£¶?¯¼˜µÆÎ?'UÍ£¶?ïÑÒ$ûb?xº5É '
?wízêE?xº5É '
?åê¿'7â?ÌmüÕ¤?Ô+æ€Û=?ÌmüÕ¤?î9æD†Ül?¡Å=ž\|!?¬a›´">?¡Å=ž\|!?ä™N_€æg?µ^HåRþË?ÖÍc@þ32?µ^HåRþËAGN4FGL J1012.3-1232¿ãâ¦[|†@ARÒ^Ý)À:Ž-–;@HÀ<Rv'=\'@̀½)Áš@l dŽõÒ?Àƒ­Éý9§¿¢ûä"ºü&?á Ÿiè&@˜&+ô¿"Ów¤É›¿éÓïk]F,¿çç	Ĥà¿æ¿¸èz0¿æ›}Ëú¿®04âF÷AGNbcuPKS B1009-123?ïü-x-?2'WwàL?>—;G3-D?2'WwàL?ïñå!Ϫð?\Ìï'X¼‰?\5¼7nÐD?\Ìï'X¼‰?ïà0]Q%?jÙjG¥
Ê?oÏ¢¬3.?jÙjG¥
Ê?ïö×ù·Í?:¥Ë›o"?RPÊ4ß?:¥Ë›o"?ïørmŽVx?Pv…ä¢(Ï?N6J(e¡?Pv…ä¢(Ï?ïÀ-ª]6<?€íœÜ]N;?é*µè(?€íœÜ]N;?ïÑ'Yð?{k¸ôŸm?wp7LQÐ?{k¸ôŸm?ï¢æů¢?wÚg
˜Õ?‡F{Õ§?wÚg
˜ÕAGN4FGL J1012.3+0629¿ÃØT"*‹^@G~´À9v¹Ù«À;Ù;,ü¸M@ú£è'M?ÿ"~b®–?²äv6¾/?·åøÂÉé™@ëíœP-?@fŠŒ¶\H¿àÙCӔ¿ãsˆÃˆ€m¿Þæ×¥mã2¿á!‰¢«'¿áò] D-¬¿éçšät«AGNbll3FGL J1012.2+0631NRAO 350?ïþuÌWS?"Æô¶Iª?/H¡b%…?"Æô¶Iª?ïï¡x‹,?añNù˜ á?`^‡'Q?añNù˜ á?ïó-h\Ï~?_
äª è?Y¥/\^"¬?_
äª è?ï㞊f˜2?N@¦©9ä?lau³"Õÿ?N@¦©9ä?ïü½=:?8Îøݾí²??*pŽT4?8Îøݾí²?ï¯Ê#‹[¤?'5ª¢
X?"
wy*â?'5ª¢
X?ïæƒ%Ӓþ?téÀçÓò?i|Ùí41ô?téÀçÓò?ïozâm©?|,no⢊?'£ÁY´Ï?|,no⢊AGN4FGL J1012.7+4228?ᝒwë©@K4ohÜÀ:hÙÒnÍ=À<v½ôµ@ Žòµ¿•?ükWfï"?Àš<VÈ? A>â?á/WK@鄈»Oø?ïä]ý⎿æܬ1&é¿àö>"þ¿Ì¨µUⵗ¿áÍ)HÎ¥ë¿ØüŸxUÒAGNagn3FGL J1012.7+4229B3 1009+427?ïþྤɁ?wfßÍ €?!ô?ì`?wfßÍ €?ï÷£Ñ¤G?RS&Ýç?P¸^W+'z?RS&Ýç?ïú¯Ë¬ˆ¬?0kã»j<?E@Ј€Ó?0kã»j<?ïöèàåħ?7ï8U5?R.=сóL?7ï8U5?ïþ˜'©yG?_'0Hž?&wÙ¢Vó˜?_'0Hž?ïÜöƒaŽ?vÌĦz?q"žŸb½W?vÌĦz?ïü{²í—a?C"MI–'?<"hU²[?C"MI–'?ïí»oàÁ)?LÛÕÍ0
™?bDNý?LÛÕÍ0
™AGN4FGL J1012.7+2439?í ¿jäzh@K0ñ€
|[À8¥î'):ŒÀ;ç(Ag©]@µÐÍbsé@ZA*2?¤.OÊkI?Á¼£´Ð'@æ<à[@aÓNq'?¡-àõ	¿àlh'î¿ãàoa6Ñ£¿æt -œñ=¿ì‡!œ1ú¿ïÿûÞ]BüAGNfsrq3FGL J1012.6+2439MG2 J101241+2439?ïí<[¥î?dÅâðÌ£?bä,·€?dÅâðÌ£?ïï5‰ñþ,?e·´QI?`ÊvCd?e·´QI?î3ÛáV‹l?Ÿ×!ºdë<?¬ÂAës0B?Ÿ×!ºdë<?ïùµô@>?:ëʏʝ?I(/l÷ì®?:ëʏʝ?ïÒbÆHÏ'?xLd0Mõ?vΜëf ˆ?xLd0Mõ?ï¬Y7À?'Ö?¯pÛ?"ûi¿Í
?'Ö?¯pÛ?î¯dÅ㊻?œ'"þ¨?¥	³¥6ðR?œ'"þ¨?ïåì¦åe(?\d±…Ë"?jYCÖ(?\d±…Ë"AGN4FGL J1013.3-2551?ïð¸Ú|Å@8Â÷ÓÀ:¬l){À<L-ë˕•@Œ	K¬Ò@'óUÎ?̚Ïú~¶¿?á=ö¬m²@ø"5´í³@eyœÞ?~[lƒr¿à×ϔþ)f¿èxQJuo¿î|?k¥À¿ïÿÿ" 5•?ïìÝxìzèAGNbcuPKS B1010-255?ìxËû»€?¾M?
†ü3?¼9§è"#ý?¾M?
†ü3?ì†nçò˘?Àpy~Šä?»ÌˆÀi£C?Àpy~Šä?ëA`^©G{?©–B"Rœ€?Âú~…Zâ?©–B"Rœ€?î™ÝºcqG?'!h…z}Ë?¦b$YÈëŽ?'!h…z}Ë?ê(ïËWµ?ÇRҏXš?Ç\CÀÒ¡+?ÇRҏXš?Îù%}4€ˆ?Í·úأŗ?èA¶ ²ßÞ?Í·úأŗ?ái†õ¨†?¶Ê×5p?Ý,òÞ®õ?¶Ê×5p?ÝèB³r¢y?ÁX°"Ìš?áÞ¦F®Ä?ÁX°"ÌšMIXED4FGL J1013.4-4006¿í¦,µÊ<@*ÆÜ~ñw§À:z6ó²äÀ<VL¹6£@]U¼ú@â@ÐO8?Õ7¹«?Á§ßÐ?ýxZŸˆÆã@Aï"¿ïðõkQ‡²?ïmÅÖ8†Y¿å[¿¤Q¿Ûìü=3g¿ä\°ºv¿ïÿø¨ó©°AGNbll3FGL J1013.4-4008NVSS J101319-400549?ïûԗúæ™?5™iՖl?@­ŸýÛ^•?5™iՖl?ïÔ–€›­?|×í5y¾Æ?uô´Õ¯©a?|×í5y¾Æ?ïê¨0qs?n»UÿÚvõ?eWÏq°-?n»UÿÚvõ?ïÚ'ñ¶'!?UúËÀFL?rì)‹‡?UúËÀFL?ïêºn®çè?b'êþ?eE'NXgõ?b'êþ?ï£^†›?§ À\)‹:?ŸË"6¯ô¸?§ À\)‹:?ïÓW5z?{oϏ­"?vpýB‡KP?{oϏ­"?ï#‹‹õþ0?‹Ko‰¢¢?›ŽŽza?‹Ko‰¢¢AGN4FGL J1013.7+3444¿Ì-oD0††@KÉë têŽÀ:2Ÿ|àÀ<o©æ÷n@,­c%`@!þÍ?¹?½CW¾ä?ÀoU®2X@YO?Ù@R5£zîß¿Ó3ўm¾Ê¿æwÏz&6Ë¿åÙ¾bPØ
¿êÀÄyA4¿ï÷?œÎ€?Âø<èÎdAGNfsrq3FGL J1013.5+3440OL 318?ïþð!2!?"ý©æø¬?/°ü¹î?"ý©æø¬?ïö¼÷U?R^à¦?£?R‡ßèv?R^à¦?£?ï꽔†Æi?aY5ŠØ3ÿ?eBkpú†Ÿ?aY5ŠØ3ÿ?ïó£¼2?Eš+7*×w?YÛÞ[;ì?Eš+7*×w?ïøOìÞ?IEXp‰X?NÃçŽ}Ð?IEXp‰X?ïÖnÊ<¶?uZÿèK?tÈór	?uZÿèK?ïÝþhPKr?rƒïß?qËöÖß?rƒïß?ï¶-ÓÅ0ï?rBÊhæÊ?'t‹p?rBÊhæÊAGN4FGL J1014.3+4112¿ïÕ¼Ì	êv@K{š¿4À:'7褙¨À<"þ)f+@{"Œ¿k@	ÒaaCè?¸ºt_Mm¿²æ I»O?ön"¸‰Hé@$Ž³°F¿æZùý‡€¿ãŒ¢~š¿æÈZý|˜¿á7ÏÆl`¿ä"'É›À¿ïú®‡ggîAGNbcu3FGL J1014.2+4115GB6 J1014+4112?ïþx7c{?oJλ?(|‹··2ë?oJλ?ïö;d@Wš?RóœQ}HÈ?S‰6û_Ì_?RóœQ}HÈ?ïôçÞv‰?TË£€šé?V0BÚ}"?TË£€šé?ïø'#?4馘V‹?Mû«?4馘V‹?ïþ}Œ¦I´?!ø+•áhÖ?('2ºv?!ø+•áhÖ?ïØk×>•½?tëºÿ¿ñ!?sÊPæí ?tëºÿ¿ñ!?ïóK€ÿ;V?^ª÷uyø?Yhþ'º¢ƒ?^ª÷uyø?ï'hÅ2Ç?p
‰òÜÓ?~¶Ë›V؉?p
‰òÜÓAGN4FGL J1014.7+3210?ïñd³Ö(8@Kâ­>'À;[HŽå
±À<ÓESÇ'q@ x|l75Ì?ö»Ò©…Ÿè?ÙV»"«P¦?ØmAKúªV@cS;ç6Û@¤tz{FG¿è…¶Æ'¿éÛÐ`U*T¿Ü€("X"¿¿¯'ÿ'¿âVbýüÁ¿ç½®(`qAGNbcuNVSS J101445+320725?ïþ,îB	Ý?"©sëE?-1?,¦?"©sëE?ïö_ñéM?R×瞼nˆ?S@F"÷@?R×瞼nˆ?ïÝ҆ӡÜ?b½g1x…?q¼"ob&?b½g1x…?ï÷ò›F¨?7/¤T²¸m?PÉpº¢l?7/¤T²¸m?ïþ¤vJÐ?"›É"N»Þ?%¸—¸MKÔ?"›É"N»Þ?ïÐÏÚæI?ŠK£éêïì?w˜u"[–?ŠK£éêïì?ïífתC?oÖãe»R?b™é8µN?oÖãe»R?ïç¡ÆÝ?Z{¡í>G?h^:ÀZÝ?Z{¡í>GAGN4FGL J1014.8+2257¿îA˸m÷@K7=áâއÀ9þ†åÀ<XnoId@=!¤W
@Ũ¹?º,Ö¢¹}æ?³yHÁ9ñ"?ò…×Û(@ûRK§HY¿ÊœdzÓÜ¿åfâÂØWE¿é¬u>p~¿ïφ»p"?àË1¡ã•¿ðAGNfsrq2FGL J1014.1+2306OL 220?ïÆ®ÓÆÜ?°Ô°Ìø?|¨–9 ]È?°Ô°Ìø?ïôÄRÕ»?X™®ïJ?WÚwŸ¹ç?X™®ïJ?ï]›è@?Žãðژô?"Lž"´?Žãðژô?ïüD5Ráé?3ˆ*W¦x?=ÞU–?3ˆ*W¦x?ïæHòLj?vfUw"Mè?i·
ú'Îf?vfUw"Mè?ï³Su??Žsƒ,F°?ƒ+?g±2?Žsƒ,F°?î£]ˆyê/?žCú
Ÿ;I?¥Ê'v©?žCú
Ÿ;I?ï¿ëmKÝÏ?}鿇L"?€$¤q†M?}鿇L"AGN4FGL J1014.8-0537¿î'ìxRà@Cúãq*À;û
͹\À<'@eJÝt@¸'r0@=ø{§@K?˹€ôM?¹Ç‡þç|&?íî/ªèv@hÚPCs?íÑóbb˧¿Ù3œÆtÄ¿è@ ìߑ˿Üñ±Þ‰ã™¿ë;<¡Æä«¿ðAGNbcuAT20G J101446-054049?ïü×é­Ð€?."ß2²ªd?9@³@Nˆ?."ß2²ªd?ïñ>Še…Q?]põ•~»ø?]'ê¹Cno?]põ•~»ø?ïÜ ¨ºI?m
Ì/?q¯ø¯wˆ?m
Ì/?ïëºN×Ö?DÙ¨"f†?dE±3ïé®?DÙ¨"f†?ïüª)@8?6^lèU…?:«˜
tW?6^lèU…?ïÃòÒ[?"Ë.Údä?~ø£3r?"Ë.Údä?ïÜ_Úä›(?yHF0Q´?qС 'Ã?yHF0Q´?ï  Z9B¨?r
8Ý53?‡×én?º?r
8Ý53AGN4FGL J1014.9-4508?îƒÓ'Ai@"Ùº=À:VR,†À<5'Í»à@	#Îç.M@bE¿ý±q?¹‰M-ZV?¬½™P?ò_äÓSÐ@)Ó)]F'?×ÅUŸ™¸Î?ëàÜ^e;¿äV$ßÞL|¿è°d‰Ø[¿Ö}ÓLKˆ¿ä¼†~3â†AGNbcu3FGL J1015.2-4512PMN J1014-4508?ïöÔ
;…p?LøñB²o¢?RWågøà›?LøñB²o¢?ïÕéÅ<Eè?~S', b?uA¸Y?~S', b?ïÁ§©?}^ŒµÛ?{ôül{Â?}^ŒµÛ?ïáë•9ã|?T—§™'ç?njÓÚô]?T—§™'ç?ïÉXBP n?qo?QôDX?{SÞ÷Œ1?qo?QôDX?îÀ5z!b?¯y+á–n¨?£ü®©lÝ?¯y+á–n¨?ïl\å箃?'rœ@;>?'tcC
/ž?'rœ@;>?ïZçÖ#Ê?ƒÙ˜"¦<"?"¾c¾¾?ƒÙ˜"¦<"AGN4FGL J1015.0+4926¿âN
Bøg@J[9&A³À7!ÄÐoÀ:ùxiž)K@¸>Öªq-?ûþ/Egé?ŠžÔí?¥ç¨ß÷eÁ@WØåó@Yy&1—þ¿¶!x˘Å3¿ÔñëÀ-@¿ÛOqtõ¿Ú"fÝ.ĺ¿àޕÜär¿ØñnØ$ï¤AGNbll3FGL J1015.0+49251H 1013+498?ïüVGŠX3?;«‹:îŠ?=MÅ»èê¤?;«‹:îŠ?ïöù¯ü)?Så,#NU¥?Sæk͞N?Så,#NU¥?ïÊ6=é©?—2Äõ?zäáW§"y?—2Äõ?ïú[Iìvû?5'ÔÐNƒÆ?F'Ù %̖?5'ÔÐNƒÆ?ïþ¢ROÙ?&%ÕÛºLò?.%ݖL…k?&%ÕÛºLò?ïÍþÿ¶`?íÚсÄ9?y€
(ÜC?íÚсÄ9?ïä®â½5?{aËÁó̉?kÿQ3@J¦?{aËÁó̉?ïöŒq=?Eqó;ç+Ý?RçþêŠ?Eqó;ç+ÝAGN4FGL J1015.6+5553?㓪ú•@HûìÃã?À:`"ՔÀ<®¬&dØ@vÀ7=.	@Óû¶Å$?¼3Øt »Í?¾šNʓb?þÞüz9'@ñµh'?ïõd›‹a¿ÕUšü›¥¿è2ø6#¿åEŸ¶´2¿ïÿv½Ì~É¿Î$¡Š~ɊAGNfsrq3FGL J1016.1+5555TXS 1012+560?ïü:ºªÐ?7›'»žÏ?>*)÷`?7›'»žÏ?ïöjÆÙ~ó?UƒJF¥ùË?S*rs}¹´?UƒJF¥ùË?ïÑ#äê-Ž?vR^FU?wn
:Œà?vR^FU?ïñˆ›_ö?EŸÛA'o?\ïÎÁ<?EŸÛA'o?ïøƱ•?K¦t+Â?LçìË)ˆ­?K¦t+Â?ïٞI©8?w c‹`?s0Û/]0?w c‹`?ï¶aÖ´­?'óöc÷Y¿?'gŠH…å9?'óöc÷Y¿?ïÈB–þ^À?hQùÎ^Ü}?{Þ´œMÅ?hQùÎ^Ü}AGN4FGL J1016.0+0512¿ã¸™5_w#@Gƒ*ZFsÀ9Ó¬ºÞŽÀ;ô{/PP@/Ô®Bž
@¿û}º@?§Å#yñw?Œ¥'ÛÃ?ãŠ
jKÎ5@ÇÑb³©e?ï k°RBÿãxQ [ª¡¿æpÒÐòÌ;¿ày7Ó¬¿âAØ}7¿ê'õ¦	êeAGNfsrq3FGL J1016.0+0513TXS 1013+054?ïþ",SVO?°''1ôl?&Í<9׬†?°''1ôl?ïõrŠƒsŠ?Yü±#‹"?UꐤÌ×?Yü±#‹"?ïø>Bä^Â?<(½äïø?Oõ,/ev?<(½äïø?ïÿå*3&À>âál³Íä>êÕòi#8Ù>âál³Íä?ïþÉd™ì?A¥)D¶D?#i¼âqË?A¥)D¶D?ïÛ¯ŸP¤?qOˆ?rq¨Jj+?qOˆ?ï÷Î`Ô3Ò?V!¯ráÙU?Pc>~ûæ?V!¯ráÙU?ïÿîp$€>àUòþ€>áëÃé"zÁ>àUòþ€AGN4FGL J1016.4+7703?ނºytF@BmÏÝ"…fÀ<€Ä"(ï
À=§s³VB@!À˜ÐÆ×j?øêܝ$h•?áŸ!"OX?ï2€áü}@	å¨ÃÙD@ÐEìO¿ïÿ.ÿqå¡¿×2ê£whí?ïÔ*pìÒ¿¯ÓÏAé{Ñ¿ÙÕõ?‡ªY¿ïÿùŸé"ÚAGNbcu1RXS J101647.6+770239?î¥yßj\?½­¦õU`?¥¨bÏ4?½­¦õU`?ïuo׏"©?¤ø˜Øk¡?'RWœâ?¤ø˜Øk¡?íІ mž>?¦IœƒSÊ?±{ÊûI3'?¦IœƒSÊ?îaéh}± ?"íñMÀ?©áiyܳ÷?"íñMÀ?ïÄuSäk?"úð ¹ÞÞ?}ÅVoN®?"úð ¹ÞÞ?îjGÓÿ?¸ÂÁeæcÍ?©^{ó¹	?¸ÂÁeæcÍ?î{½WmX?Ù^õ\M?¨D.|@ø?Ù^õ\M?ê¡Ö;áWž?·M™í¦?Åx§z¡‡?·M™í¦AGN4FGL J1016.5-2650?ÕY†^m7@8oawêiÀ;2üÁ‡À<¥D@¡°¿@ ýçP[¸
?ÿ'6¾ØîC?Ôï˜ß_vˆ?ζ`dCÌ^?õr-å˜î?ý:¥¸‹Í(?î'ØÚø¿ïøžwNëö?ïÿ¡Ö~ý6¿Å¾´Ü?,¿ìè=Öû#ø?»¯d9ÕåAGNbcu3FGL J1016.9-2653NVSS J101634-265057?ïٜû'¡Ç?jÉ*Um?s1''Pg?jÉ*Um?ïԔŽº9ð?€ü²8»ú?uµ¸¾_è?€ü²8»ú?ïa¯}0­G?‡î2AQÌ?"ÊTÂí(?‡î2AQÌ?ïSÛ-|~Å?"H['"‰?•"šSßÃM?"H['"‰?ïâÙÒÕá…?f{ƒ8¯æ?m&-$Ÿb?f{ƒ8¯æ?ô¢ºç?Ÿý;ڕ›?ßBÍrc?Ÿý;ڕ›?îþIŸ†Õ?•\þa.? o7¿`³?•\þa.?í¢ÊKNn3?¤­0]í{V?²é­¥šæ?¤­0]í{VAGN4FGL J1017.3+5204¿ÛÏj湚@Iü¦\ö{À;†ì"øø¥À=š‹1!
@ ¦ß¢ú@?úpŽX÷ˆ?ÓCâb¶-¤?ÔÄO»)6Z?ûj÷	·8ç?ù&¹Ã_¿ßW7õ9Ó?á£&`;ÿà¿°Xߕ&mR¿Öƒb¯É¿à¨Ž"'Ùd¿éҜŸÞW9AGNbcu7C 1013+5217?ïø^nîS?D$r&¹x?N‡ÿ¢6Š?D$r&¹x?ïÇñf	IU?|TÎÌ
+?|L﬩¡?|TÎÌ
+?ヤ¤¬%?w2ù÷…6¦?€ZÖߤ­?w2ù÷…6¦?ï&ÓIϽÿ?v8nШœ?›%–Ìçx?v8nШœ?ïókÆ]Ù
?R<V>óR??Y(s 'û€?R<V>óR??ï,ß*·'Ž?¤Þåàq?šd¢;ÖO?¤Þåàq?ï¾j'2¬?ƒ‹™¾¼ðŠ?€e[T\Ÿ"?ƒ‹™¾¼ðŠ?ìÁMDgŸ?›¢ÉPèç?¹÷-•ÜÃ?›¢ÉPèçAGN4FGL J1017.4+2538?äÙ÷5^º(@KÏ\WìÀ;Î²€À<ʴĘJå@#mükJü©?ñxá'ͤc?Ù~íEé]?Úu$²?@Áù£Åm@¬3ÁM'°?ï»U
ôOÉ¿ïæòåˆ[¿ïÿè«î0?ïÿülò¿ßÙ%ÀÙÏj?Þ"ø!å-AGNbcuNVSS J101724+253955?ïû¥%F"?<*†r2ã%?Akiø½ÉÎ?<*†r2ã%?ïóï'·÷J?^W/Á€"Ã?X!°^<f?^W/Á€"Ã?ïō÷¶·?x³ú"c…p?}9F¡P"?x³ú"c…p?ïö¸ý™?L‡‡QphÊ?SàŽ$5^p?L‡‡QphÊ?ïú:š@ï›?R«.ÛÍS*?G–΢À?R«.ÛÍS*?ïϖR‰²?€(ósÑÈ?x4Ö¢iÆö?€(ósÑÈ?ï·cª°~t?…&k=.?''`îç?…&k=.?ïÙ@&û[D?t•m%ÏrÆ?s_ìk¤ñî?t•m%ÏrÆAGN4FGL J1017.8+0715¿Ôïm#¹™@HGÐ|"µÝÀ:´ÿK¥À<N°ªWVÿ@·ê)))@ÎɟâÚ?ÉIO>ׁ1?¹þ_ýý­|?ì>m=ðüW@
QÃu‹~?ïûŒž"#¿ç?*¸:o¿èÒ¤Uµ>¿èiʞõ#¿ïô£
[£•¿ãú'®š²žAGNbcuGB6 J1018+0715?ïþ"3íÝ?ÅÎéYæ?&¼ÂôaJ¾?ÅÎéYæ?ïô†8$÷?Tï8ìŠt9?VóT×RÏ?Tï8ìŠt9?ïå'H?fù·^¢?jm¸9ux?fù·^¢?ïñÑü.Ä?D¦N1ò–?\\Â1s?D¦N1ò–?ïÿ‡¸Í?Ä4Îá|?8KEžÌµ?Ä4Îá|?ïÊ|B›°ö?ò:Ÿ­Ã?zÁÞÊä´Ý?ò:Ÿ­Ã?ïë§Ëáji?m+£˜[6?dX4:w0?m+£˜[6?ï©:"óÖ?qPh:`ñ?…±{'š{?qPh:`ñAGN4FGL J1018.1+1905¿ç"G¸{\@KÉÙÓEÀ:xàU¬ÛÀ<"eByø@FOo©Ü@˜0LÎæ?¹F½S³{¿ d¬Á®Ox?æîÆؤ@	rmœ™ì¿Ù·
bZé¿åçZíŒ_õ¿áá›@bƟ¿åP—&ø'M¿Ëªø;»lþ¿áTHÏAGNbll3FGL J1018.1+1904NVSS J101808+190614?ïþ€'úè6?SÜ'¶
ê?'ý|qº:'?SÜ'¶
ê?ïöžì%ð?U°Í3˜<†?RÂ'/)p_?U°Í3˜<†?ïøYM‰ ?S~yȺä®?N›•éÞÊ?S~yȺä®?ïþoåC?5||ºh?)±¸v·î?5||ºh?ïýYçŸXm?/%¢Dà?50ÄU¯ño?/%¢Dà?ïØt+²­?ußþüÌy(?sÅêC}°?ußþüÌy(?ïú´{'ë?P"/LsÌ?E.XÇÝÚ?P"/LsÌ?ïùŸv'y—?='ñ}ç¯U?I'(/(ºâ?='ñ}ç¯UAGN4FGL J1018.3-3124¿ÅN?ö]@5ÕW2À9´¸ÙÐÁÀ;òŒVºø@zõ }ùÖ@°1;nÉ?ª
¹|
¿?®ƒ
¶è4@	Wɱ@iDû‡ H¿ºNnxƿᦕ€…K"¿è¸Ëž#—	¿ç×"'$€¿ì3bƒþ¿ïÿò(¦è7AGNfsrq3FGL J1018.4-3119PKS 1016-311?ïõ?Jÿ¾Î?M¡UoæÒ?UjU¸´?M¡UoæÒ?ïëTyZ4?s¥ÀÒÄ6¿?d«pLì\R?s¥ÀÒÄ6¿?ïÄò>\˜C?p~ù÷Oœ¾?}†àéÁ"•?p~ù÷Oœ¾?ïúxtIÃ?3îÕ>OÌ?Gò\×<È?3îÕ>OÌ?ïõ-Ilä
?R»`"³hã?U¥lô½‡+?R»`"³hã?ï‡Êª'A9?™/š²Z?Ž
Uin!©?™/š²Z?ï±1xöv?…ïu©§
?ƒ³¡ãÙŒ?…ïu©§
?ïâ‰IaÀ1?^æ¹'d'?mv¶cT?^æ¹'d'AGN4FGL J1018.4+3540?ïýebÁ|@L=
à"S.À9ÌQþ'BÀ<i­1üÒN@ðÇP6#S@G³zì/i?µÕRWeÂ}?»8­ªÑ$?ÿ»ê&z@±~Rû¿ËžM]€ä—¿áݑ`eŒ¿è« —ºœI¿æ@>-b9¿ïWàyQû¿ï•ÂH"AGNfsrq3FGL J1018.3+3542B2 1015+35B?ïý'P`Pß?%yØ£å?3m~HmG?%yØ£å?ï÷]0Õq?P Ätqi?QEÝ
އ?P Ätqi?ï癚xð4?g#KQ"Ÿ˜?hfef‹Ê?g#KQ"Ÿ˜?ïü¿Å8•?)åÍÖôêÇ?:Ø%¹¾0?)åÍÖôêÇ?ïþG‰Š
Ž?!È°Ùð?+‡dùÐv?!È°Ùð?ïØLÚú ?x	¼1ît?sْt‹"?x	¼1ît?ïì›êVËi?g¯Ðøm÷?cd¦tç:?g¯Ðøm÷?ï÷ÕlÈD?E!®'µ(£?QÄU9­Gº?E!®'µ(£AGN4FGL J1018.4+0528¿ÜÈÙo"Úº@GÕËeè'À:,ßØBKÕÀ<öó4@O-\¯ƒ@uð¥)?ÂN…7x'?¸¨*ÕÁ"?öš۸ù@†ü®'ÎI¿î¡¢7_é?ïö€Z-s¿ä
Ÿ¥Í/¿åÓsD›:"¿áŒ	XnV¿ï¬¿EûŒÔAGNfsrq3FGL J1018.5+0530TXS 1015+057?ïþ*O´É ?&†¾Q·?-[û r?&†¾Q·?ïô`4Ñ¡{?YÍ\ª¯ð?W?–%ÃIq?YÍ\ª¯ð?ïèMηU?j;Y"ìõ?g²1lfâ	?j;Y"ìõ?ïö'N€?;ܸ$ø+3?RÜå–kÀ"?;ܸ$ø+3?ïúi•Åσ?@£‰À‡;í?FY¨¨o¬™?@£‰À‡;í?ïÈQé4j?ŠÎU,$!?{óW*RFÆ?ŠÎU,$!?ï½5GyU?ƒæ÷ ­|?€½ò¼¥?ƒæ÷ ­|?ïМ	áUE?k}¤/D0?w±û&²µ_?k}¤/D0AGN4FGL J1018.8+5913?éM:ì@HIÚßµÝÀ:›&Š®DÀ<Ì_‹€Ò"@¥¿â®‹?ÿ•a%´Å?ÀòBÒãg?¾o/êÖ?ÿk/=Û,â@{Ùs¤<‹¿Êk¯¦vKâ?ì	ÒÄ]"¿âvIh(ÞF¿à©RtA}¿ßˆn ¿ïÿþBe«+AGNbll3FGL J1018.8+5913TXS 1015+594?ïûGÇê»?Bõk¦šÒg?CâßÜL?Ý?Bõk¦šÒg?ïìŠ/eÁ?bÊJr‡4|?cøuü•?'?bÊJr‡4|?ïëX¶á?h.½`PÖ?d€§kzˆ˜?h.½`PÖ?藺ùæ"?gñ³îMà¼?†Áx¼Çu?gñ³îMà¼?ïì["#³¹?f03Ånz'?c¤lw?f03Ånz'?ïµáyé6K?…¡ùy#
"?'‡¡±-'?…¡ùy#
"?ïÙn×à7t?z™§¼¶ú?sH"ÿf&?z™§¼¶ú?î3æ{8t?óûȊ^B?¦üÁšF¸?óûȊ^BAGN4FGL J1018.9+1043¿è?Vx÷Qu@IMæ`ɊÀ:ÆIéXÎÀ<f,§þ·+@Éáš9R@·S´Eí?ÑĬ{*C?½è""¨¿?én
ŸOæó@—©Tw¦¿äÔ§Awï{¿èôúþ¹Xý¿èú³$…‡¿ìÛÄanYû¿ð?ïÿ—ŸïI$AGNbcuSDSS J101857.97+103625.6?ïüQ½ü"?:ubI'ng?;õq€%â?:ubI'ng?ïï&èïe?bÑÞ҄Vò?`þØï5#™?bÑÞ҄Vò?ï¸kÛ	??Xܽ7E?ù$øgš@?Xܽ7E?ïöµ[
,?Cx1oÜ­P?R•J1ØçL?Cx1oÜ­P?ïý§C·v
?=™˜ij?2Åä¶y?=™˜ij?ï‹2>R? °vLj?3zþ9[Š? °vLj?ï¹­º|¬é?'Ú*â6€?"'W5Ýç?'Ú*â6€?ïwl²þ
?‡'D(Óý¦?'i™^¦Î?‡'D(Óý¦AGN4FGL J1019.7+6321¿Õ®çé!°ï@G % …²À:h!È`À<'ž1Ún@‡-nÎõ?ÿ
ýÌ=[?¼]Ú{·?ÉgÒa·*#@؎6F@"‹½¸Þ?îísk1§B¿Í¶†9j"Ù¿ÞMdºã¿áŸ°9F¿æ˜f^ꖿðAGNbll3FGL J1020.0+6323GB6 J1019+6319?ïîõ¹€â?Y²Â†·œ?a
Fyæ€?Y²Â†·œ?ïñ %†Ä¢?[®ôù]?]¿´kÆj?[®ôù]?勞,'ü?"vùñ?†Ô4öø£?"vùñ?ïÍ_XÍmÿ?Y'ú#Sãs?yPS'¹Üž?Y'ú#Sãs?ïá›m{¥à?km¯OMÅ?nd'c]à?km¯OMÅ?ïÃÂYx¹?~ƒáçà%O?~Ó^p%'?~ƒáçà%O?îcæÊ#û? ¨Ës'ïä?©Á"Yt̗? ¨Ës'ïä?ïHgƒP?|¼XÂV*?–ý¦œ?|¼XÂV*AGN4FGL J1019.7+0511?Ã0Рt‡Å@Gâك"t—À:áüjIJÀ<pšäó4@@ Œ£jRÚ?þú¢
¢?ËÌÆÐ&?¶IÏAq9~?íM	""}Ì@
!N§-¿Ø©Ý´{/¿æÀaïß Œ?¡x­™W¿ÖÞ¾fØ|-¿Ú<XüŸ£¿ê<þޗÐlAGNbcuNVSS J101948+051327?ïÿƒ5Û?_ÜFÌÍ?2¬jaû?_ÜFÌÍ?ïõãÎéT?T]^¨s{t?T8b®‰2t?T]^¨s{t?ïù»'LTS?S÷¸~>?I»4c$ä?S÷¸~>?ïýgŸÔú¡?fZA‡çB?4ÂÿYþ'æ?fZA‡çB?ïÿ²oÔNK>ûr¢–vg?dEà€í>ûr¢–vg?ïÒ؁$Çy?zslÔט?v"¿mœCK?zslÔט?ïû±btO™?[~Í3þ â?A:u-Hì?[~Í3þ â?ïø³…~¼?@BsȒä>?M1éVë—?@BsȒä>AGN4FGL J1020.7-3920¿î&V—w'˜@-¥ê«%)À:õgXÔ­lÀ<"UàÝ%
@ dæÃC?þ*™Eå½?Ê÷ JÂÌ?½Ù!™Ø®­?ôä$7í'@ÜÛNšÂ¹¿ïÜ>Å7­?ïâÉ¾²¿àِ"Š¼¿ÍOÿ‡4<H¿æEz=]Ùz¿ä¥ ¸ò¥AGNbcu2MASS J10203893-3920563?ïþ´rQÅß?à+0çWe?$¸ÖÁç?à+0çWe?ïà†÷óÓ?s©`v¹K
?oyáïNüð?s©`v¹K
?ïó'MÍ?U$¥%ñY?XÝ`òÅð?U$¥%ñY?ïá‹ÃYB?Q'/~.w?ntöþÍƊ?Q'/~.w?ïþk*ùÜX? —fÜè]?)MSî¢? —fÜè]?ï?KÄÆæP?¡V•Y‹:?˜‡j'Ññ?¡V•Y‹:?ïõÖ&'¼?c#j7}?TÞT#·°?c#j7}?ïmî:ä5'?Mï(?'B8¦è÷ ?Mï(AGN4FGL J1021.1+1626¿ã€Ñ9v¡Ð@JÕQa£ÊÀ;cüÈ=À<ÇG&/>²@ Ô±šA_F?ýàA8¯sö?Ó? ^¯¸À?¥Ïƒºþ?Ëáºö¶€@nÊ£|ÇQ¿ïÿÇ*Ì\e?ïÿ<‹¡‰R¿æ‡9zu$¿Ã¢ÓÔþÊv¿å­å˜îy¿Õ¯=oÍAGNbllSDSS J102100.35+162554.0?ïþéà-ý"?YKÏ"?!aû1^þ°?YKÏ"?ïôӘ‡ºŽ?WÖ­w2Ä?VXÏXÿÛ?WÖ­w2Ä?ïîL¨"÷2?e\W&R>?a³WVN
?e\W&R>?ïóWËZ'?@æMí6"?YPxŸM/?@æMí6"?ïÿ-j|³?uO"±\D?R¿ÜÖb[?uO"±\D?ïÒ2´!"?w8.ý'ä5?væ¥û›$?w8.ý'ä5?ïðR电j?m|ë-?_Z0­YÛb?m|ë-?ïʌóâ?n`
¬DýÅ?z¹†d¶ƒ?n`
¬DýÅAGN4FGL J1021.4+8021¿Ôi»ý¾ÿ|@AM˜ˆøbÀ:W‡¦RÀ<˜ƒÛÂ3@"¸_˜@vWu1ÛD?»î›~¡Â?ÅӊV/·@~ɄBð@?üo5JÁå¿Ú¶ÇÝyÃ:¿ßWsÄÈÇZ¿ãd.]‹vk¿ãºPþöſ×øz?Ϟîm0…AGNbcu3FGL J1021.8+8023NVSS J102201+802350?ïœs±'ª¿?‹RcÝLJC?ˆã¤çDa?‹RcÝLJC?ïÇ3¹H"?~Ý\Ds?ŒŽ3>>ý?~Ý\Ds?îžÓGî´²?™X(‡žõm?¦Ë|É1ë?™X(‡žõm?íýŠƒÐã?•Í<æ
±1?°¯Û'é?•Í<æ
±1?ê‰úX¨?Àç—ð2hÄ?ǝØ®b?Àç—ð2hÄ?ëeËׇt?Â×S+©¯š?ÂhУñâ0?Â×S+©¯š?ënK[.`!?®âªA£¬?ÂFғF|?®âªA£¬?äoæuóÖ?º•¾‡B]?×!æ3U?º•¾‡B]AGN4FGL J1021.9+5123?¨O\šÆÑq@Jt×I''?À;҃9LÀ=Š'¥aN@ƒ{³žÇ?õ¢Œ¢:R?擥cÒ7p?ä³øà¦ôK@¸d"@úø´‡0¶?徚À
F«¿âs1fªY¿ÞçÂòXx¿Î û;;¿êFJ'Û¿ïâ~
ÇÚAGNbllMS 1019.0+5139?ïÛ×-ñ!b?o?lÀ†ç?ri Üj¹?o?lÀ†ç?ïâœZœ·9?r'5B '?mc¥ghO?r'5B '?îÿD–‡ìH?'®+•è±›? ¶šð×z?'®+•è±›?ï}msËÔª?sM/°â(†?RQp­?sM/°â(†?ïy¤Æ•Èv?Ý°í=ô?Ëg(‡C?Ý°í=ô?ï¯aºZ.u?‡Qyã(«?"''b•*Ý?‡Qyã(«?î"E)"?›tÔÉzÆ?§¾k°ß"¾?›tÔÉzÆ?î¡|çÝ?—ª9‡=Õ?¥è1"ÁÍ?—ª9‡=ÕAGN4FGL J1022.4-4231?è 06©ŠR@(¶Žæ¸0^À:\a5¤ý{À<^~ø-£§@4Ö ˆŒ@ª"£hO?ÀºIýÏùþ?µÏ?Š?öFB‰èK®?þ¤ŸÔò
I¿ÜÅÄDèè6¿Øä2"Œ—(¿äU.enâ¿á=u×H¿â°T[¡çF¿çYº¼)›AGNbll3FGL J1022.3-4234PMN J1022-4232?ïùcdz?Kë'öPå?JrpÒa ?Kë'öPå?ïȼ.;t?"ˆ"IÁ?{¡èàæ?"ˆ"IÁ?ïïœÀ†?Y>Æ{°=¶?`c@Äñ¨?Y>Æ{°=¶?ïÐ'Ïk§]?Wt'€£?wì;	µ?Wt'€£?ïîÍŠz©?V*®|B,^?a2ÿ[hO*?V*®|B,^?îDCXx?¬?C¯7?¦+»Ñš}?¬?C¯7?ïå@Wo8Ù?v'×|OÈ?j¿¨¨$~¿?v'×|OÈ?î³öB£#í?Ž®–v''>?¤À›ÕÍÁ-?Ž®–v''>AGN4FGL J1022.7-0112?ïhžH™»—@F08⟜éÀ9˜püÀ<Sq@€bÐãå?þY·+zØ?²ã2½—{?¥(+Ã'\?ó{–^{¶Z@ôœ"µâ{¿äÓF=üåÄ¿á¹\þØ<¿Þ2½—z°¿Úv7_ÞO¿à‹aÝ냿ßä€]2‹AGNbll3FGL J1022.8-0113RX J1022.7-0112?ïüð¥ˆÔê?,©óM ?8zÔs)ô±?,©óM ?ïòÑaîÜ?^¤]Çû:?Z]<œÂ†¶?^¤]Çû:?ïõ€,¶}?Rý¡eÒ?Tÿ§ÅEz?Rý¡eÒ?ïç"ÃIsð?RJÊâèq1?hl<{rÈc?RJÊâèq1?ïù~¿=`?>m£üªž?JÿpfÊ?>m£üªž?ï½<ìšrˆ?•N7/
¬?€°ÄÖK¸#?•N7/
¬?ïêÞüWÝj?rB""MMÚ?e!ƒÎ?rB""MMÚ?ï¥|áI}ð?um§§*@?† Ç± ?um§§*@AGN4FGL J1023.1+3949?Æÿ&ˆ¢Gà@Lo1½èÀ8ßÉ#ÊàdÀ<"àæ_E
@ŒÊ(W¸@ùÅS[È?¤L/¿œsÐ?»'Æ€FP5@ä­Ýô<}@ü9§¿Ì†ùXñÞª¿áíÁ9ÓÁ¿ä'ÙaÏ©¿éDåw¾}¿æV†''>¿ïÿúŒ—ÓAGNfsrq3FGL J1023.1+39524C +40.25?ïüqWR™¢?<µŽ°"Cª?<uFšª¡?<µŽ°"Cª?ïö"=Žù$?YOƒi51"?S»"Š¸Z?YOƒi51"?ïˌҥ˜š?~ŧ>Eԁ?z9–´êß?~ŧ>Eԁ?ïÿ×Ä«Ù>è®òµ½îÊ>ô–YñÎ>è®òµ½îÊ?ïþç<BY?'Žš?!Œ>`™?'Žš?ïغY‹?A?w<—ýaü?s¢Ó0ÁwZ?w<—ýaü?ïÚ*¶ël©?}qÄíË$?rê¤yŸÄ?}qÄíË$?ïÿ½_^>ù¯/§öŽ?¨E2ÁÑï>ù¯/§öŽAGN4FGL J1023.2+2859?ï9U¯	@L²82vtÑÀ:ªÐ»nÖwÀ<Œdý±@xšô¬·@uX'?ÏÕ£5#Î;?Ï?/*ee?þˆýՃU@™½Uá]þ¿Ú0œ_ǐοÝ&‹º³Å•¿åâ,m®"¿í½mHضæ¿ÚØïþ¯¿ðAGNfsrqTXS 1020+292?ïÞ'ÞÉØ?œf݆q?pì³Ñ.)?œf݆q?ïð¬ÞÎ_¨?]Ñ°Š?•1?^¦Aí!ˆ?]Ñ°Š?•1?ï—JçÚÅ3?…†"‰]þ?Š-F¾O=?…†"‰]þ?ïìm3ªÂ?L‡ùDGi?c'Ì»üæ0?L‡ùDGi?ïø¤®—úÕ?MêÏ&ð?MmDû´(?MêÏ&ð?ï²´Z~ë?Ž…óeL?ƒxÒæø‹,?Ž…óeL?î`¼ãöŠ? ÈÔ1Õl?©ô1½'Ã\? ÈÔ1Õl?ïYì"ðaŸ?†ÕñeB?"ÂohÓ?†ÕñeBAGN4FGL J1023.8+3002¿â\8Ì5‰@LÍ®>lLYÀ;)€z䢬À<µb+nBÔ@!7¡¬ãx?ý´òd/U?Ç}ÖZHŒ?n­àMˆ?·¸Ñî×@€Qû,Ý?ëÔD$òþ¿ç³VÚh¶¿æg¾U:Å¿ÒÙ~ —O<¿Ô¢ÃäÆ¿¿à§".ÍüAGNbll3FGL J1023.7+3000RX J1023.6+3001?ïÿ_›	õç?µÅ½#´í?¦#O?µÅ½#´í?ï÷^*zw?Qގ$Q,?QC«'ã?Qގ$Q,?ïûbÚÉB\?-ô¬[PX?Bt•Ä@µ?-ô¬[PX?ïý˜†
 ?"ÓÎG¦?3;ÏßÞÇ?"ÓÎG¦?ïÿ˜œC˜>þrëÁÁV'?	Øþ÷&¨>þrëÁÁV'?ïØàå;6@?w-ۆ'9¾?s'H?w-ۆ'9¾?ïýÆÿD?AÛù6†
?7Èd">•?AÛù6†
?ïøÛNxf¢?>Ÿ|_úè?L'Åo'óë?>Ÿ|_úèAGN4FGL J1023.8-4335?ï¾nš^ÝÓ@'3ó.ZÀ9"Üõ)À;¸•Ew–@ 
½Ál‡?ù¬gíO#T?°9?硏\?¼ßyLȼ@ º}>ð@¥['¡'­?ï÷=Bÿ¿‹â꬗ß@¿Í/?ɸ3¿×•)<ºEŒ¿×úžAI!¿ÜÞ&¼W^·AGNbll3FGL J1023.9-4335RX J1023.9-4336?ïûŸ±b?DÖ@~?CˆéOÎQÊ?DÖ@~?ïƕÀh‡Ë?‰Y¨È¬?|µÂ2t?‰Y¨È¬?ïÐ:¾J†•?zTs½™€~?wâ ¼€%ä?zTs½™€~?ïÜ1.KAó?Uäø£yq"?qçhÖïj¥?Uäø£yq"?ïøšß¥þ"?M'ìÑ,8?M"£òå?M'ìÑ,8?ë#œ_?²Šc²â'î?§¥ÁPYï?²Šc²â'î?ïѨI	ß?"-ö†¥8C?ww+ð¸P?"-ö†¥8C?Ò6:œ?xÚ÷\îB"?ŽÒo½?xÚ÷\îB"AGN4FGL J1023.9-3236?ï÷ø5A'@4½Þß)À9høH{™ÔÀ<h;R¼@ÕÈ<DSí@Yú—á2µ?°¡ŸL‹ôÀ?¼ODyׇ@ "Ú@¬Ûù Ý¿Óå•ñnlÅ¿âã}_*Þ¿ç‹1÷ÉЙ¿å¨âaßn¿è¤Pwؕ¿ïÿ܎᯳AGNfsrq3FGL J1024.1-3232PKS 1021-323?ïý¥\_@?+–l¬¬w?72Ö!›˜?+–l¬¬w?ïñA³ÿvm?h×ØæØÞö?]|˜Põ\?h×ØæØÞö?ïã+šß?pÿ¬¡rÑ»?lÔfÚPj?pÿ¬¡rÑ»?ïÿ­r	>ôŸÉD‡Œ?£i/‰L>ôŸÉD‡Œ?ïü÷ÛKô(?05«Þ÷kÁ?8A$0¢æ?05«Þ÷kÁ?ï¾4IrÇ?†(L̃Ë?€rí¸s²&?†(L̃Ë?ᆭ25‡?;€Ê@܎?€Vy#LtD?;€Ê@܎?ïÿ4Àžb¤?«˜Ü_?gëRå?«˜Ü_AGN4FGL J1024.8+2332¿î8Œ¨3T/@Lf/¾3¬ÖÀ:Jº))À<'ÜÜåHÅ@ex?V×þ@Ë\ŠD'?¹ÁHà®ø?z™™øÛ?¿¹:^J¹@0g…JW<¿žóÂbe¦¿çy€‰þ#¿â˜ ˆ5Ä¿çJ†¡oPñ¿è_ÊÀØøª¿ç_·¼]êAGNbll3FGL J1025.1+2333MG2 J102456+2332?ïàð£?­þùŽ¯'P?oð¸5MV?­þùŽ¯'P?ïöÌé/ây?Tþ–óõÏ0?Rf-êrœÏ?Tþ–óõÏ0?ïêEá>Q?iÁ¤EÛ?epºF&L?iÁ¤EÛ?ïò•+JÜr?E‡îÒpÒ?ZÕ©¡@ÛQ?E‡îÒpÒ?ïèlˆòàæ?f®Z¦~¬F?g"væ£yù?f®Z¦~¬F?ï؝¹Êø?u÷ûNa?s±#$҅9?u÷ûNa?ïÉäÛ¿âa?ƒƒšŒMI?{
'`#r?ƒƒšŒMI?ïϑD#ñ?fxYÞ?x7rûz«1?fxYÞAGN4FGL J1026.9+0608?à±iR:F@HãBEõ­—À;éuyÿ À<…/PO¤@"êvÖËÿ?úG«<#?Ƨ0›~K5?™:"£§?Ó/á»vc?ýÄL`*ã¿éøÍ ¯¢ð¿ï—eýŠÚº?èËb¿gßb¿åÉ8Þmß?
^b`ó5¿Ï¸fGÐAGNbll3FGL J1027.0+0609NVSS J102703+060934?ïþ";[ »?h_v?&ÌGy¦®?h_v?ïôHO,Áˆ?]ï¬kÈl?WobòP/?]ï¬kÈl?ïîñˆKœ?QÇâ0Ñùñ?awÀ" ?QÇâ0Ñùñ?ïø'ŸTo??{çvœ"î?O½¶xøª´??{çvœ"î?ïý^Sâ)?/éAƒy"?5
a®‡]?/éAƒy"?ïÐ+"\e ?y‹½Q€?wên³àh?y‹½Q€?ï{(ô?jÖ"¯ü-?ac²1ãù?jÖ"¯ü-?ïås³ð¡­?e¶©5H*I?jŒL9ùzÈ?e¶©5H*IAGN4FGL J1026.9-1749¿ï†Œå"@@',ºs-õÀ8ýN.KmÀ;ށOøÄ@¦'¥¸‹?þ™‹Ýtk?¨ý?l®?Ÿ-ڃě%?ôÈØ앿ð@œÜ$¾¡?ïÿ"­~ÿ¿âöq ~¥¢¿Üœïd|Vh¿ÜÂܾ²W׿ߣÂèG|–¿á[íœP-?AGNbll3FGL J1026.9-17501RXS J102658.5-174905?ïþú+Ϊ?4˜fK	? ^1NÒÒ=?4˜fK	?ïõ8ÓJH?Uq"Uc?UŽY‡vO"?Uq"Uc?ïò ÝõWõ?f_NË9V½?Z¾DrÅu8?f_NË9V½?ïþ´—æë?æá\O¿À?$¶'6U´Ñ?æá\O¿À?ïÿê-?±}P
K?=YøF&é?±}P
K?ïÓä¾'Þ?v‹uÂy‹?v
 Ñký?v‹uÂy‹?ïê{±§,?tO8>¹8?e"NQ%?tO8>¹8?ïþ'|®k'?£x.?&è3ƧJ$?£x.AGN4FGL J1027.0-8542?Ãóû'þ'À7£é·¿ŽÀ9VFíû¾À;äé@- .Q?û£®@˃?±«bï¹`ß?´×mÌ ª@PÕ¥¹b?ë@­3J¿ÕTF=Ñò¦¿à@GD¿ÛQ'Ã'ë¿ÔÁä×Ût¿à(»àì?¿ÜœŠâAGNbll3FGL J1026.4-8542PKS 1029-85?ïò!Õ¼­?\Š3å%¯J?[¼UˆT=?\Š3å%¯J?í—\y8â0?¶F/8w¡¿?³E7ð¼~?¶F/8w¡¿?ï%kæǹ?•)õÎë¹?›Rƒ#™3Ù?•)õÎë¹?í‡7¥ÄÜO?—	Àzn'?³ÆBÒµ‰?—	Àzn'?ïÓAQó¬y?wuÇ^Â?v_W%?&?wuÇ^Â?àjz~§J?ÑÒUÆÛò?ß+ò±k?ÑÒUÆÛò?ïä½âׯ?""U'wðÑ?œƒhE\Ø(?""U'wðÑ?â_l0C®o?»CÉÀã?ÛA'Ÿx£!?»CÉÀãAGN4FGL J1027.2+7427¿íUÖ.S9@Cšù jn3À9Pý^e%À<gŒSã@rªuÛy@;'}E¥ü?°F[®ýY?µFÏóî@g‰¿1×@.[~?ëÖz•ÈSÁ¿ÚOŒ…4î¿æ!pÞ9†´¿äñ"íjÒ¿è…?\ŒH¿ëKã-abAGNbcu3FGL J1026.5+7423GB6 J1027+7428?ïþ-${_r?®'{γ?--¸GÕïx?®'{γ?ï÷$j 7á?S?P%?Q·+ž"ýA?S?P%?ï努#»­?nÙæb	?juUëbšÅ?nÙæb	?ïû>â
n?/Æw–#ƒ±?A‹…"·¯?/Æw–#ƒ±?ïúA&æÉ£?@{\½j§€?Fûe0Ï+?@{\½j§€?ïÜg̏\¡?rñú_S`ô?qÌšŽ?rñú_S`ô?ï©E6s?†CÆVЗ?…®²iûðr?†CÆVЗ?ïôÿLë"ã?Jßâ.?VeÆ{[?Jßâ.AGN4FGL J1027.6+6317?؂C«j@T@G}"M:"À:;ðJ€VÒÀ<¢w$ú‹L@²' V!J?þS¢úkk‰?¸ø*We?ª®NÝ]¾¢?ðïga8)<@lïåU¯µ?ïû=ù_ÒÎ?–'¿§í'¶¿ä¹xýAߞ¿Ñ>sV¿áƀ,‹#¿ëùsôÄb›AGNbll3FGL J1027.7+6316RX J1027.4+6317?ïûM²Õº?<wŠcðÿ?BÉ4ÔØeÛ?<wŠcðÿ?ïñ…R?^Krā
?]ÊõÆcü¨?^Krā
?ï籸?qŽZ!ÿ?hÿNµ0Ø?qŽZ!ÿ?ï™P©öÅ?pu¾QÙÙ?‰«úGÃÞÉ?pu¾QÙÙ?ïöè
¯ 0?IùŽIR»?R/ꘀ?IùŽIR»?ï΁ž-ێ?wãEQÉAl?x¿0ú@Dá?wãEQÉAl?ïá•XŽ®Ñ?zÛz¤0ØW?nj§ƒ/&Œ?zÛz¤0ØW?îÙíí·[ª?Œ!nI:¯Ê?¢a! >Âf?Œ!nI:¯ÊAGN4FGL J1027.6+1828?ïÿ6²LK'@Kñ«ó8qaÀ:zXËs0yÀ<u¡Å¸•@œ_.
Ú@ÕIe¤Ÿ‡?¹ÎAÒ¿ªê^ƒ"â?ð­
ê¤@є\Ãп×wCÃÏ"=¿é"iÐË¿èӓZ»7y¿Û¢ëý¿ˆì¿ããðj`Æê¿ðAGNbcu3FGL J1028.0+1829GB6 J1027+1831?ïú4ªè²˜?<ÅWNa?G-S¢Jâa?<ÅWNa?ïð7œ¾+
?]§™³¯Q?_Æÿ[Ôã?]§™³¯Q?ïß}Qm
¨?p, üñ
?pAWU'×ç?p, üñ
?ïëCdtI?LÑGÐ_@?d¼àVӇ?LÑGÐ_@?ï÷´ßg¦z?I3qÞ+Ã?P–A¸«?I3qÞ+Ã?ïº4õ"Ó?Š'YÔ?rßòt¡E?Š'YÔ?ïÊ6Üy×Ì?PÓ2f·t?zä'Äsñï?PÓ2f·t?ï?Æ7w?ˆÒÔ!¢l?˜9!-?ˆÒÔ!¢lAGN4FGL J1027.6+8251¿äßäÆW'@@hó¡LìBÀ:Ž‡=vƒÀ<¾|ŽÆØ@^Ç»ëÓù@é']e5å?¼±]Z¤k¿ò»Úó<^?Ôå¢;~±6@-W&,¿ã{ŒhX®î¿àèh~ïtB¿äiæ÷mŠ¿æ<Ý5Мe¿áe¥«ö"p¿âÖ ž9%AGNbcu3FGL J1027.8+82532MASS J10284195+8253398?ïþnfKI¼?)žIh³?)™@/|?)žIh³?ï÷U3Z—É?TUÁà+?QU™t¾Æ?TUÁà+?ïöçiŸð?DW‹ÉlÔ6?R1,ùØP"?DW‹ÉlÔ6?ïþ§0¹?ýΆ¨Ï?/E'Šeõ?ýΆ¨Ï?ïý7´ÞTÆ?2	·ÒÌí?6BZÝXBÕ?2	·ÒÌí?ïؔR‹=?vc½NˆƒÝ?sµÿÂÌ¥?vc½NˆƒÝ?ïóOsìÇû?fÍ« U-?YaÎz
V?fÍ« U-?ïùQxv;ú?;Y†Pò‰x?JºÒf…?;Y†Pò‰xAGN4FGL J1027.9+0252¿ïýù¶ïì@HÏÃøÀ:nӕ=êFÀ<A†l–+P@³¡ÀY¡Ý@õ±…H©½?¿ÿ²RM)Ô¿µ
…†H?ò¡öKKX?øâ£8SÙq¿ãa|¢¿ëZ¶ÐE®¿ìÐHbz¥¿¶d±Z€¿êê~äa"¿ïïK|ÖtAGNfsrqTXS 1025+031?ïñË«å	?^W©Ô_N?\hª#*­£?^W©Ô_N?ïU=@A(?£×FÁcÖ?•_xY¯©
?£×FÁcÖ?ïqÁI¢Ó?•"ûÁ›°?'ÇÖÛÓ׬?•"ûÁ›°?O÷æS?mõKŽLH(?€Ôr‰J?mõKŽLH(?ïpÏBjU+?˜g¿ˆ¿Í?'æ¹"'?˜g¿ˆ¿Í?ëJcÖ¿ý?Ç©ÿ–+X§?ÂÖp¥°?Ç©ÿ–+X§?ïX[é,KZ?'›x?"ô'ÕO*Ê?'›x?ë'ª^?µA·Y*æ?Ù÷©UŠ‡?µA·Y*æAGN4FGL J1028.3+3108¿áMu@MOп "`À; ³	­'ìÀ<Â=U™@óF3@@÷U^×%ì?ÁÁŒ|Ћ¿—».>׬$?ÖÄzÃÀ‰@	¢ohî€ý?ècÆ
•ê¸¿¯Ù1½šÞF¿ç,$K8ãv¿á*`üš¿çN£Îç?È8ôhG<*AGNbllTXS 1025+313?ïÿ°Ú?²pϕáÍ?ßãM?²pϕáÍ?ï÷"@–óø?Q£»Šç?P÷HJŸž?Q£»Šç?ïö&>û_Õ?Tâ VAÂ!?S³'?´?Tâ VAÂ!?ïüÊÅý-? ýú#jß?9¯;êÙQ'? ýú#jß?ïþmìl¥E?"†º0Y÷ð?)!=;.?"†º0Y÷ð?ïØÀ—E'˜?uÒö»r¯?sŸ´i•L-?uÒö»r¯?ïôJR'&¼?c$ƒ1!²?WkZh?¨6?c$ƒ1!²?ïô-c\é?F€<7ó*?W¥9££Rg?F€<7ó*AGN4FGL J1028.4-0234¿ï‹€á@FB[åÙäÀ:",Ý®œ`À<YZ;µ¸´@œ±a;.@}G{¿"ÿ?¼9ï:
?´«§Ž#ïž?õ	Ggž@
Õd]͐—?ãi§c†¸¿åvæF–"¿è2ŒÖ<¸¿çwlþ°õ¿ìð]ºpT¿ïñÈdˆ?ÕAGNfsrq3FGL J1028.5-0235PMN J1028-0237?ïü"!c»?*Ü®ÈOÌ?;fòÏJ`±?*Ü®ÈOÌ?ïô±`ñÍ?Z»dUy3?V=ρ¥?Z»dUy3?ïíhOìô­?L¡á»"†î?b—°/è
û?L¡á»"†î?ïöÉ0=¾?;Ø»Ùb™í?Rm 4¦Ð?;Ø»Ùb™í?ïü€(
³?5Þ?Œ†O?;ÿ~¼Eþ¤?5Þ?Œ†O?ïÆܨѵ?'©˜ó´ö ?|ð'¾Ôõ?'©˜ó´ö ?ïóNF½‡=?\ð¹Ô-ë?Ycrâfå,?\ð¹Ô-ë?ïÜòsÇÅH?^8ÿâ¹;?q†Åý0ßõ?^8ÿâ¹;AGN4FGL J1030.2-8403¿æÛ¿â"	À6:îA'šÈÀ:Ë£jÓ³qÀ<t±i@ k篧"@Â9櫛$?ŝ´†YöÁ?³Îð"{rg?ñBºtÛt/@Š²öâË¿ïÏAò×?ïýw$#Ë·¿ç	Ü!Ôf¿ãØҔŒê¿Þl¤Ùh¼'¿ä.1,edAGNbcu2FGL J1032.9-8401PMN J1030-8402?ïýÆ£N4}?#æ6vÈû?1Êæ•$ %?#æ6vÈû?ïí¬Ÿküº?críþ3ÃÅ?bS`ÆÝ~/?críþ3ÃÅ?ïê$ý̅:?g8Ï-¹ú?eÛû!-Ö?g8Ï-¹ú?ïè ú"?Pªû9œV×?gpßÊ)&8?Pªû9œV×?ïúó½7¿›?:_"È¢ˆ˜?D1®×Ù1?:_"È¢ˆ˜?ïžÎåßK?6\0Î2?ˆLFvÿ2G?6\0Î2?ï䕺M)?v xúsiP?kjE¥f?v xúsiP?ïKÀÓøé?ˆ°ÍÂßñ¿?–‡å}wîÝ?ˆ°ÍÂßñ¿AGN4FGL J1030.4-3001?î‡w…ȁd@7¥/Ÿ¾wÀ:—F·G*À<Wé^ÓÊî@ú#d=;@ÿ\±Ö§?ljCu –
?À¸SÙpõ?õ'ÐɱZ@æ¼,k˜Õ?ïyێ0¯Ë¿è"^ß´[¿çÔ/—¿æÒ"!=¿ïÿ­_I;³?î47ûäAGNbcuPMN J1030-3004?ïò‡É"æ&?SڒLd,Þ?ZðlE,?SڒLd,Þ?ïÝ5ëtWÁ?w$¸ä"?qe
U¢S'?w$¸ä"?ïÂÇúc?tìx¾Ì'»?~œÛ¾x?tìx¾Ì'»?ïÐMÍé,?bÄ.Y`ï±?wÙ‰Hˆ?bÄ.Y`ï±?ïÓ¯%X:e?t¦Ÿ"—ë†?v(mZ"?t¦Ÿ"—ë†?ï+e¸§¸?§*q­<DÇ?šœóCß?§*q­<DÇ?ïwš;ˆŸÕ?‹Àg¯Sϒ?'¸‰Ä›m?‹Àg¯Sϒ?î(%ÿæL?œfr*	¬?­£q79?œfr*	¬AGN4FGL J1030.6-2028?ï(Èÿ@?s̪ï,À9䌎\À<.'"ø@ ]>6q?ûm±cºº|?ÀªQø›1Ê?º¸p^â¹s?þӊ¦·N@:㫶}¿å<O;§uû¿Ýg"s—§¿Ý–±Ý³$¿Ðkž3²4¿Õî¯á»v¿çø
¢gÉAGNbll3FGL J1030.4-2030NVSS J103040-203032?ïýßJŠÃ?R" ó3uš?1¨Îãào?R" ó3uš?ïôE³N²§?WÙ¬Qª´?Wt™"Òß?WÙ¬Qª´?ïò3µÓм?n"v±aˆB?[˜"äë¨ã?n"v±aˆB?ï÷S®Z?4R"±G.å?QX£×Iv@?4R"±G.å?ïýC2b[r?)ðz¯5Ù,?5æl,ºMb?)ðz¯5Ù,?ïϱyñCá?u±¶Ôçp6?x'BôÐ+¼?u±¶Ôçp6?ïäœG?|Æàÿ¨¤÷?kóc¼tYS?|Æàÿ¨¤÷?ïâY+ó×[?[Sºlû¾?m¦ÓøêÔÌ?[Sºlû¾AGN4FGL J1031.1+7442¿äzDÃ@C™b¶®}À9×â[ªJÂÀ<7 Àiçû@ÒÛ¯"¬@j¶ÂŸLa?°/x""]¿ž¶eà¸À?ð_1£æúu@;ö%`¸¿Ú«Ä"o
¿ãóVµ{¿äÁ߇Oj¿ä¹mtw¡¿å°‡‡H^>¿'fU8Z~@AGNbll3FGL J1031.0+7440S5 1027+74?ïþcAæ Ó?ýz-ðô?)Ëä±2âš?ýz-ðô?ïöç"wã*?R'rª&»?R0öá~û«?R'rª&»?ï÷-¢¿Kõ?\L`u'2?Q¤ºš%FÀ?\L`u'2?ïù)°It?5óªÊq?KY?/bµÏ?5óªÊq?ïýaŠ…?,·N¾y?4÷ëÛí³?,·N¾y?ïÛD¾T?qyTœÍ?r]õª—½Ô?qyTœÍ?ïõÌ}qšÍ?hâG}®Æ?Tg|ÿu?hâG}®Æ?ïä¨Y'?Zž0uz>?kW÷©íiB?Zž0uz>AGN4FGL J1031.3+5053¿Õßåø[µ¢@K:\|ؙÀ9$wSôsÛÀ;ñEgée@ 'äõ8?úÑW%€Ã	?¨â¢:ìª?¦ÝäIk.@Ûh‹Ú"6@{Û3íÃ=¿ëdµ÷ž1¯?±¡ÙY"0,¿Ú¬)Ür\¿ÓÂNĉ1¿ßYvɋ¿¾|^pÐAGNbll3FGL J1031.2+50531ES 1028+511?ïý"'¿·?&Â;wT¥Ñ?3^Ãʏ™²?&Â;wT¥Ñ?ïòH‡á¾Õ?XN•-
H?[nïäŒVš?XN•-
H?ïí_XCý ?jì óš1ë?b §õ»Ð?jì óš1ë?ïºkPu?hÔèWËK¡?%Nj•?hÔèWËK¡?ïú6¡ôÿ=?AAwúw|?G%wûu«?AAwúw|?ïÍêJiÿ?wdڋqè?y
Û¸¼K?wdڋqè?ïêV u«Ô?s¢äÍpÊç?e©_†4¤X?s¢äÍpÊç?ïSà/ˆ·?‡î±6žâ?•ƒý~…?‡î±6žâAGN4FGL J1031.6+6019¿à"ù)´@HïÝëÙÀ9qÊ0:ZoÀ;ßþiýʜ@}'î°@ח{²(?³ dd?¡A¸~ƒ‹?ìEHßlâ@/]K4²¿Ç,ý6¡þ¿åh9Úí!¿æ9ÐÁN‰¿çk%@@¿èT@ßn:¿ðAGNfsrq3FGL J1031.6+6021TXS 1028+605?ïþ£8mŸ? ÑQŸbŽô?.E̕¼qE? ÑQŸbŽô?ïø	ŌͿ?P?£Q™n?OØê.Ÿ?P?£Q™n?ïëY<²7ö?Q|yïw5?d¦Ã٘?Q|yïw5?ïþö/zJ?sBè*bL?.П½¡â?sBè*bL?ïü`g,F?5õ®Œñ#?<üÆ#ƒgŸ?5õ®Œñ#?ïÝþãËA?qËÍ5äљ?qŽ3̘š?qËÍ5äљ?ï˔z9ƺ?{œ,½¢‰?z5Âìžõ?{œ,½¢‰?ïú൦¯F?9çð"N²?D})¢Õ'è?9çð"N²AGN4FGL J1031.8-2609¿è"€ˆ¯;@;ÚÂXՄÀ;bÍÞDÄUÀ<©EW"&@!"«s5Ø?ÿUdìã2?ÉRß äçv¿'õžþ'U?Ëò{Gžû@=Ü.""?ïÿå(
eC¿é#´ùàV¿å"…fîW¿ÞTÊ\°¿Ùö¢½.ʿ͘uWEMAGNbcuNVSS J103137-260715?ïýý1?#;%!Ÿ"?0‡Ër<s?#;%!Ÿ"?ïôuéø<ù?WÍ©W`õ?W,3AýM?WÍ©W`õ?ïòøkÈ6K?WËá2Z?Z(j	d?WËá2Z?ïú€°eÊ?.FàÎ.?EýˆærØ?.FàÎ.?ïþÜs«?×?æ2 jp]?"8Èöþ6Þ?æ2 jp]?ïÏé€rè;?}©‹Wù"?x?⸮G?}©‹Wù"?ïõŠS*Ÿf?cËt‰Ê°?TëYÈýÄ?cËt‰Ê°?ïãD£Ñ‰~?`\wƒ{ìQ?l»\m¯R?`\wƒ{ìQAGN4FGL J1032.6+3737¿Þ/YÁ´¸%@M‹ÐÐgŒÀ9ÞHÈÆ­ÏÀ<O[ïêß@nf'†*@°ÔcšL?·٘b7¿}ËކÒz?DzvÊ·ž½@	Â*úÕsº¿ïðÝî]@M?ïû¾½?'¿ã.$5inY¿ß:;֚׿ã/×^ G¿ÚºTDzÙ:AGNbll3FGL J1032.7+3735B3 1029+378?ïþ¾åŒþ?ú÷Ôpd?$§`€…?ú÷Ôpd?ï÷¢R>ªú?QQ1ÏDœ?P»[õ›Û?QQ1ÏDœ?ïö'{ü«?B›C:•v]?Rû	»ˆ‰S?B›C:•v]?ïö«BŽoð?AmKyãóÎ?R©zþ6?AmKyãóÎ?ïýU¯p+È?/Š¡&bõ?5R†oœny?/Š¡&bõ?ïÛá+Ý¥?v¨`˜ò?rjd£qÍ?v¨`˜ò?ïïcêÒ-?k)ïçÕÎë?`œü×TÛ½?k)ïçÕÎë?ïéqðՍ?^ÑÚJˆ=<?fŽ'³HÒ?^ÑÚJˆ=<AGN4FGL J1032.7+6624¿ìÏí
è~@F¦ˆabñgÀ:³Ò†ëAÀ<áN‡Lü@Ýòd@;bŸ1‰?Á-蛊_•?¶á@w>{?ó{X|˜Ø@&©b"?èø±Eˆ¿än"½"u˜¿Ü§A¼c¿â¿Sg†¿ä?_¼S-¿è?¸¢HiÑAGNbll3FGL J1032.5+66232MASS J10323905+6623234?ïþ!áxÅ?)´ƒ\úŠ[?-æþ%G™'?)´ƒ\úŠ[?ïõ®>'"*?WJRÅô?T£ƒHcŒè?WJRÅô?ïøšêì6c?Iô•@'
9?M"S€ýã½?Iô•@'
9?ïèÝK]³?J5ýÃÄZà?g"ðèÜ]?J5ýÃÄZà?ïý*åÄ?*ÿúåœÝ?3–ª•h¹º?*ÿúåœÝ?ïØ[Dãù~?u[!S!¡?sÒ]¥`˜å?u[!S!¡?ïú
ãÊ?`»Ïf"ã?G˧ýc|w?`»Ïf"ã?ï¾bî¯'?f–¢Í)¨î?€gDT',T?f–¢Í)¨îAGN4FGL J1033.1+4115?ºª™= –Û@M0){úLbÀ9ÖÃƓÎÀ<T²¡¨[Ô@¼®Ç~.@¢Ÿ§Ñ?£Û1ƒIÛ?¤ÚT¼ÅÄ?û¹St[@Úº±AV?×6
G¿àĽÛB[¿çŠèáÖIM¿â±ªÂ‹Ö8¿ëÁ+Cz©¿ïùá½õ™uAGNfsrq3FGL J1033.2+4116S4 1030+41?ïý6ëHÞ?*S¿×ºÿ?6H©¡nÔ}?*S¿×ºÿ?ïø'?i2°?MÝF¨Ó©^?M»û/Üÿ?MÝF¨Ó©^?ïÜèÈDÁ•?tÀDւ-ñ?q‹›×oé¡?tÀDւ-ñ?ïùo:‹Œ?@$x¿oØÄ?JC¼¤»?@$x¿oØÄ?ïýdñµÿ?/üæžñ;?4Øsƒä0V?/üæžñ;?ïÝïŒ{Š?såWµ?quˆ;"î?såWµ?ïÞ +Ùø"?vQû	È?p¯ê
Ä­Û?vQû	È?ïô!ofÑ?V¿@Èt.ð?W½ô»}íà?V¿@Èt.ðAGN4FGL J1033.5-5035?à¿Z/:D
@×ÙõÀ9¦œë]±ŒÀ;êÅ®ËZ@ Ü:Óær?ù4m)Ï?»t#ùYs?ÉŒv›gÐ@¸Íi@Yùb¼c¿èõµ>:Î2¿Ûª7áî?µÖãÑ÷,¿Ï¢ô¡¨î¿âÏW xEŒ¿âAºÃ.¾AGNbcu3FGL J1033.4-50352MASS J10333216-5035287?ê0Ë|•§È?Ò±Ä0µÄ?Ç<Ò
©`â?Ò±Ä0µÄ?ï
","ªê?¢‡HÍèð^?žMzf‹jÑ?¢‡HÍèð^?îè%œ'é:?•Ÿ\ZÞ?¡}¦;AY?•Ÿ\ZÞ?ïlÁJýC&?swÍ¢¥ÓÚ?'g֛01F?swÍ¢¥ÓÚ?éGÕà$v?Ãw­˜v{T?Ë¢à¨n(?Ãw­˜v{T?érV;Bm°?ÊÄvBª^?Ê6§öI??ÊÄvBª^?ëΛØÒÙE?¬G·N¶Fy?À՜´šì?¬G·N¶Fy?í"nH¡É-? †'0íÈ@?¶ì¹9èœ? †'0íÈ@AGN4FGL J1033.5+4221?ë['T>@M{À;×`RP.ìÀ=qZ¶.ü@!gضea?ô6%UúÞX?ç`^*WÂ?ÙzH0yÿ?òµ
œ;5@Žî
å÷¿ë}Õ]¿ù«¿çÄ£2Ÿ¿ì	ۂr?ÌêžÚK:'¿Å±ÓLBβ¿î÷#"úAGNbllGB6 J1033+4222?ïü7Ú'?;ì¡1îNÈ?>A0@&Jô?;ì¡1îNÈ?ïø½xéB?O÷'ÅÁý?O©	Ó<àè?O÷'ÅÁý?ïÏ)ÃóµD?oxÝ97?xkùÚ?oxÝ97?ïþk%›x ?äôav«?)M¦":TK?äôav«?ïùTÅ%¥?SHNR'V×?J¬ê³Uk?SHNR'V×?ïÝ}ß·œ?rð
7%²?qAw£'Ó?rð
7%²?ïÆêŽdîR?"L'ÈóS?|Š¸«Üªú?"L'ÈóS?ïú– é.­?DÏØ
ü®?E§|g…?DÏØ
ü®AGN4FGL J1033.7+3708¿ïE]Ïõ@M¯Ž!–R½À:PêÔÑÀ<H™—ZÛ@»r‡[ÿ@bcQÞïå?®ì¿Uڗ¿±_2µ@3=¯÷¥@™£½‰ä¿Ý~7þÉõ¿éSFc'ŸÐ¿æȬŒ%=¿á¿ž{«¿Õ'‹Ã˜¾¿åTܛvékAGNbcuRX J1033.8+3708?ïþ*÷NV?Œû»c?-^áÎ\Jn?Œû»c?ïô?CW?T˄Ze¤¼?Wyâœ?T˄Ze¤¼?ï÷/€†¾?XÏgÛä?Q ÿòòƒô?XÏgÛä?ïò¬ÔΒ¹?B°4¨rCá?Z¦UéèMÉ?B°4¨rCá?ïúÜC|r?=@l"Ÿ?DŽòò7?=@l"Ÿ?ïÉï¢1:,?}®dÀH?{/OeÉ?}®dÀH?ïäø'z{?t——æÚø±?kn€¥
?t——æÚø±?ï~žSg±?ítâÒ1?>,,üé?ítâÒ1AGN4FGL J1033.9+6050¿ïÁ«ãaþg@HŽé_ªŠƒÀ7åŸËmÀ;B`	UX@?6̛@ÚÝ0È?›'Z¦®?¸ÈºI½c@ g»/ìVÖ@æ­Øë¿¿Ñâb
a-¿Û'Ã'ë¿âøÎ}¦ôÌ¿ã[+硺¿æ~±='ˆ¿ë‹µ±÷	AGNFSRQ3FGL J1033.8+6051S4 1030+61?ïùe™â¿¨?D÷û'È›?Ji—Ö <y?D÷û'È›?ïé\ÚoN?p<•âFÝè?f£&*J"+?p<•âFÝè?ïtB:?Êy?'¯År¢?'w¸¶Nâå?'¯År¢?ïñlÓ¬©±?SØ]˜š<Ã?]&X…°_*?SØ]˜š<Ã?ïëwÝ(±ò?`=vZà®O?dˆ#Èmn?`=vZà®O?ï¨l.Á"c?–®SyŸŠ<?…äôHØ/-?–®SyŸŠ<?ï–†Ò[q?Ž!;ÜF‰Ê?ŠÞU·÷»?Ž!;ÜF‰Ê?ï q¥ã~?z	E0†9¦?‡ã–Îõ,N?z	E0†9¦AGN4FGL J1034.0-2547¿ã[­j(_<@;—s}¦À:å
55lÀ<[€¼S@P³`•'@úњ'ç?Ð?Ÿ}3\y?º4v͒?íA".ÎI¥@¡6Æ愿ìo—!Å!³?ïü4Ï¥©¿èÞ¿¾qjQ¿Õià»[¿ïÿÙiÍy¿ïù¯æ9AGNbcuPMN J1033-2544?ïý¨³y$ë?3tˆ%U±?2ºeË?3tˆ%U±?ïðÜp¦'¿?`îìJ.š?^G=}òô?`îìJ.š?ï½$•­ô?€hz(?X=?€¶ÚŠäÍ?€hz(?X=?ïñG~LiÄ?EláIè—?]q÷iN?EláIè—?ïþ=>"¨X?.ö ÈÇ`{?,,¹½¦?.ö ÈÇ`{?ïÌãÐõPz?|µÑ¯¯\?yŽh{^?|µÑ¯¯\?ï¾Ø–‹?'ióœìÌ?€IùØ¥q_?'ióœìÌ?ï®×OÌ_Ù?x_ŸË
?"J,¾—?x_ŸË
AGN4FGL J1035.1-0608¿Ì'ò*Õ@º@E•BB…À;$=Ìê)À<m"[tšÝ@yb|¡ç@cÄ*fÛ×?ƟEÀ~ŠÊ¿…T<S~"j?»3
nmñË@–Ÿ«Ÿ7¿ïÿDN
ª
?ïû—P=Ê¿ê$½Nª‡þ¿ä†ñ i,¿Ûèù¾_!¿ïÿ§ëkôEAGNbcuNVSS J103503-061204?ïô}0éh?'NÖÛL?Wå·áú?'NÖÛL?ïóårœ…?Z½C0Æ
U?X5jºv?Z½C0Æ
U?ï­ú Æ?"&f6¹Ò?"¾OWÎj?"&f6¹Ò?ïûHl°Ž?-úûªùòÙ?BÞOÉVT?-úûªùòÙ?ïøöŒlh?R×:Ý¡.W?L%Ï@D;¸?R×:Ý¡.W?ïÃ1¶Žûd?•0²Z V?~g$Ö¾Þ?•0²Z V?ïZ÷(Q>?'r·|¿ª?"¡÷
s?'r·|¿ª?ïÛô92q?h	þˆž?rã€UÃ[?h	þˆžAGN4FGL J1035.3-2050?߁àa©@?ÎA=·ñsÀ:Õ%¹Íì‡À<'ã'÷Ó@ø'ֈ¸@Á`Dä5Ÿ?ƌÇÀ'?¤>"cì'u?ß±cÚðÑå@ ª'¹V¿Ñí¼Øc¿êo4 ñ|¯¿àµ[–ÿ‹¿àæ €~®¿ègMoœ¿ïúÒ~½uAAGNbcu2MASS J10351532-2050261?ïýõÌud?(½&,Å0?0Qžo¢"S?(½&,Å0?ïôÒOm¦w?Vhÿ¾~ºÍ?V[`¹CQ?Vhÿ¾~ºÍ?ïòšW7R?T'\Ü{}?ZËQ~'V?T'\Ü{}?ïú6´÷Í?.õöiZ/?G'ÌÖ]Á‰?.õöiZ/?ï÷{ÌÓ>?PP%"³?Q	æE]D?PP%"³?ïÓ¯"(‰?{ž«xU?v(zîÛÐ?{ž«xU?ïè9™m"›?qÃ8…ÌÂð?gÆfÊÅü›?qÃ8…ÌÂð?ïé_΂ë"?S!ØspN?f 1e·®?S!ØspNAGN4FGL J1035.3+5541¿ïɢМ\@J4…]¢r†À:ÁœiW²nÀ<¤tæY@@ß-Ím²@-î4üa?Àqç£è§õ¿dÄòÅZ?¦ŠøŸ—3?ö±
Ô~ó?îM¹kzw¿æä£î‡1¸¿è,ðùÒ¿¿á€ðя¿ïÿ³^¼£à?ïò˜Ù€9vAGNbcu3FGL J1035.2+5545GB6 J1035+5542?ïèy¡µ$˜?uxbUiÒ?g†^|UÇ£?uxbUiÒ?ïÕ	VH•?''ÌÞ°ô?uyûT+É°?''ÌÞ°ô?ï•nʖš>?"äDN{ž?Š¤MVéÔl?"äDN{ž?ïŽí^Ù?{Àk!¯zÉ?ŒD¨j[­??{Àk!¯zÉ?ïÖ隨?|–3"á*?töc¤'Ý?|–3"á*?î©ÌÝòA¯?±	¡âª?¥c2ÿþ?±	¡âª?ï" ¾T?‰e_º¬?Š÷Ð}þªã?‰e_º¬?ì
s	H?°^‡E'S5?¿¿¯$gµ¾?°^‡E'S5AGN4FGL J1035.6+4409¿äf=\èõ@Lö¸–ž=À:ó­FÈBÀ<É	<¿¤@¾_°i¿·@1"œâú6?Á¾'cò¿eBØYØ?p?¡WÝ´>6?ø¥b¥?î©?~ðöοׅ–AöD•¿è¹ƒäün{¿äùAj-›D¿Ù°}ãۇ¿í€·_þsAGNbll7C 1032+4424?ïÓ2Ë?¯@?=á?vf÷Š­o?¯@?=á?ïë²?¥(æ?jyú.
;?dMÀs"I"?jyú.
;?ï±+mäVy?ƒÖàZ³?ƒµ$wt#ë?ƒÖàZ³?ïÌî—ð¤?bé'~øð?yˆ´'û?bé'~øð?ïöãÎtJ?JÞÉØ[`K?R9ø`{´?JÞÉØ[`K?ï©D/bvË?‹¨ö;­–?…®ô£ÝC?‹¨ö;­–?ï}Kw}ª?í_)áCà?VÈyDÔ?í_)áCà?îºTs¹yù?"åŽ
'º?¤Z¸ÃŒyy?"åŽ
'ºAGN4FGL J1036.2+2202?Ö4Dþë5¡@Mw™ÅXdÀ9ãíät‰?À<oîŒ:5†@Níd	K@¾€£ÿN)?³çØýî¾ö?©ëÿ~6"?ðüÛñ¨N@J‰)4?ɶ˜ØÔ¿çL?ÿIvÁ¿ç¯9>/H¿å'^!†ú¿ïÿ΢	?ïú²œ™AGNfsrqOL 256?ïüÏô÷õ?1AG³Fãš?9‡ÆVDŽè?1AG³Fãš?ï÷—ýžb?U÷ivmÇè?PÐ ±<'?U÷ivmÇè?ïàa¿§d?qM\o"?oæž=˜ëâ?qM\o"?ïþíºY?ë%ÔÓ=?!/çm®\?ë%ÔÓ=?ïþDrºvx?)Ë$¡ ?+¸Ñu¹Tz?)Ë$¡ ?ïÙ&0…Ï?y'Éô­Gì?slç¥dTÉ?y'Éô­Gì?ïã¬Y(ª?w9¬ûtÎ?lS¦É—ˆÿ?w9¬ûtÎ?ïüdd®€\?4{(ñqŸ?<Üܦ¿àì?4{(ñqŸAGN4FGL J1036.5+1231?™£glî@KŸ8ÅCkÀ;M♽«ÈÀ<È°­²UR@ ¯pÆf¬?ù ÛýÂ8?ßËlåÜhK?Ø6Ξ31[?üäª9$
ü?ôýìðƒ¶?èy¯†ßƒ¿Þ·";8?¿â¼g#û‡Ë¿ÁJùùUÁӿ煿ý±q'¿ï÷²ß:ãAGNbllTXS 1034+128?ïð4XÕ·¶?Y")ÕöÈó?_—N;Ódô?Y")ÕöÈó?ï)ko8ó? >¢ªžÖn?šÒóЯ¡? >¢ªžÖn?ïx:ödåw?ˆp¹ð^ôÃ?ø¡6Òí&?ˆp¹ð^ôÃ?î{lÎ=ì?†Ú»±t?¨I3
h>?†Ú»±t?ïíúWR)÷?ba
ãZE?b¨Çóß?ba
ãZE?ë¾ÙLÀ?Å,̾×c ?ášÌýþ?Å,̾×c ?ïdÆ~æ ?­xS?"',³Ÿý?­xS?éäUËʪo?­®åqV?Èn¨ÐÕVD?­®åqVAGN4FGL J1036.6-3741?áFÁ!»@1äëÝ3L^À:ËƳ®ÖÀ<l$Ý/ @×è
Qé@½Ðæ7?у,$¡?Þ|7ž|ØC@Ó>ÿP3@§çC?¿©¶²"!7]¿Öš$‡¿ê¿>™Ä¿ì[1^Ƕ¿ïå¹,Ü×Ý¿äU?ÓªAGNfsrq3FGL J1037.4-3742PKS 1034-374?ïø%®Û?LTÄzè	6?Ok¬¯f?LTÄzè	6?ï§;Š3Žç?‡Æ&=Í6?†1l=*?‡Æ&=Í6?ï^Üâ{?÷{›…˜¸?">$uLª ?÷{›…˜¸?ï{˜Èõbÿ?qI1*§ò?Œææ{
?qI1*§ò?ï®;aÕÝî?‹?Î7‹&?"q'~Ùد?‹?Î7‹&?ìæôlè¥_?¿¦òâò9?¸È\—	?¿¦òâò9?î0Ö0½?ŸÂ|Óƒ?®Ü÷%0©%?ŸÂ|Óƒ?êÌßþNJ‡?¨èÜ'&Ã5?Ä̀áÕâ?¨èÜ'&Ã5AGN4FGL J1037.0-1954?æ;É]	N@@g¿rq6¤À;‡p'°H2À<¶žõ#-,@ '÷øt›]@hwhiÏ?ÊØï…忘~º£³¦?ÑM>!MØ{?ù£²½'È?éµ8%á;¿Ø×Bœ‡µ–¿éÞ@\ça¤¿Æ·¿^û
'¿é [À7?Ý¥ãߍï—AGNbcu1RXS J103657.5-195432?ïúþ‰{?=EPÐ{…?DÛº~lŒ?=EPÐ{…?ïçê˜mRF?qK꿯?hgî	‡?qK꿯?ïÒ»"‹Úâ?r^3&r?v¢66¢óB?r^3&r?ïêAaÁˆ?O­g®:ŠÁ?eç¾Ñ¯L?O­g®:ŠÁ?ïõOþ]?SvýPåÙ?UÇ`	~¦ž?SvýPåÙ?ï°b[®°?"Irù"r˜?ƒçy#ìê?"Irù"r˜?ï¹;ë,x?ÑôçaK?º±äÍø?ÑôçaK?ï[Q'S¬Ð?"{l¸ë?"•Ï°bûü?"{l¸ëAGN4FGL J1037.4-2933?æHK¡û#3@8ß ù	kºÀ9º°"rÐÀ<MÝÙe@B†øXñ@0X<×÷£?¶4J4'æ?¤$§Õ?ì4"'òÜ+@äÁp‹?î<S£C^¿åiŸš´¿æ<m8è~Ú¿à»JùùU¿èŸó»NH¿êþøcSŒoAGNfsrq3FGL J1037.0-2934PKS 1034-293?ïý<tᏎ?+ºÆ5?6Yöÿªo?+ºÆ5?ïó½<?_ÐÃN¢Ä?X…ˆ<:s?_ÐÃN¢Ä?ïñÐT–°0?WÌx.D?\_V˜æ/è?WÌx.D?ïücôŠñ?+,Uéw½É??lßö€È@?+,Uéw½É?ïøH\ÿÏ?H¢oûc?NދëRË?H¢oûc?ïÒÙ3bƒ?|ƒž$T³`?v"fVýŽö?|ƒž$T³`?ïØÎöü(ä?|Î)-ŸÅ3?s˜"wœºM?|Î)-ŸÅ3?ïö
­ÄZ?C®¤:µ¤ï?SëèTÀ\3?C®¤:µ¤ïAGN4FGL J1037.7-2822?ï¢ì¿äå@9äÚ<!~À8½ÔZ_ÇçÀ;°uÝÒ®Ž@4Ӕè@;7ÿJÎZ?¤[ã>?¸5™ióä"@oÄÖ^F@´·Ã{?¿ß3"À¼ž+¿á‹k~(Nÿ¿æn,Ε#é¿æ³¢.hž¿êx±ŒÕeù¿àšŠ?‰'ËAGNfsrq3FGL J1037.5-2821PKS B1035-281?ïúLV'*\?C·ÊÄKTU?FΤÙÉ[?C·ÊÄKTU?ïð
Â%ÔÑ?lCÄ1¿
?_ê{ùü?lCÄ1¿
?ïØŶØï›?p­€­—®Ú?s$t›¶¿?p­€­—®Ú?ïþ'¼TÑá?Ê78ëó~?'Ô9'ρ	?Ê78ëó~?ï÷Û³'ß³?KÊɬ¾F?PH˜£ç­?KÊɬ¾F?ï¾Yžp²´?"¾õeö"?€i˜Y"~ö?"¾õeö"?ïž'
¹u
?ŠhGMW²Ö?ˆv=Jŗ?ŠhGMW²Ö?ïú‰ckŠ=?9k¥ô…P$?EÚqÔ~çŠ?9k¥ô…P$AGN4FGL J1037.7+5711?ᨣÐk@Iäh3Æ*À8óz¶ƒÀ;s¦#×þ@ψ¾Õé?ü 
¡©2"?›
ß"(¹?²n+Â%©Þ@MÙ<FØ,@ rIs'r?îø^ õ-"¿ÓÕ-¤(ï¿Üw®F¥¿ÙpÜÁ·oî¿Ý{C&E¿å½•!dԖAGNbll3FGL J1037.5+5711GB6 J1037+5711?ïû;ç{"Ž??ŠúÅF÷Ÿ?Cb±¬cì??ŠúÅF÷Ÿ?ïî?Y˜]ë?h9Ññn?aÀ¦š|L;?h9Ññn?ïÖaZ&ÖÈ?}ᅄ¤k
?tÏS±£½?}ᅄ¤k
?ïãQّG?VÅÀ¡ÂÉC?l®&zÝP±?VÅÀ¡ÂÉC?ïøç)G?LÑÈ~uÂ?OÌd!~×L?LÑÈ~uÂ?ïªßåX^ç?¬>‹ÔOœ!?…Hœ)Öc?¬>‹ÔOœ!?ïà@äe‰‹?}/'ß«?o¿¸³c?}/'ß«?ï«
adÄ?rd¼%?…<§²(_.?rd¼%AGN4FGL J1038.2-2425¿âô!Š"C@=BDËáëÀ:Ž¼ôµ4À<dêúµ=d@^ou®­Ó@E$Ý/?¿á•¦'`¿žó/{Ý_Ü?ÞbyœÏ3@4J5Ù*Ô¿ÏΧBy¢-¿ç nºu\¿âŒŒÀÃ)5¿ã ¸§{Úl¿åšŸ˜·¿ïûxçrjAGNbcu3FGL J1038.0-2425NVSS J103824-242355?ïý̽™D?%ÖñLpD?1šþñƒ?%ÖñLpD?ïöW´™È?T7•ctZ?SQÒ~A?T7•ctZ?ïó–"³?[Š­ÖE?XÓڟ֚
?[Š­ÖE?ïþx|7?Sûsú?(x:<jñ?Sûsú?ïüQÅΕ?5ügý™•ê?=qЗ>Z?5ügý™•ê?ïÔç%=§*?y?iÕS?uŒmIÏã?y?iÕS?ïòµžKÉÇ?g…ð=W?Z"Ãw²ð?g…ð=W?ïúy¿ùC'?6®\³<›?Fÿ½|X.?6®\³<›AGN4FGL J1038.5+3926¿ÔPœ mÄæ@Më¦ZÀ;Â:£À<éD=F²l@%¹r@¯;Ý%àd?͎àÃy¼Ú?²–ŸOwH?æ(ä$Ø&@Q-mÌaB?ïý÷Cõ"?ëg™6Jÿ¿æ9¸RÂD´¿áuú"pmP¿ïÿõEq#?ïÿ""ÆAGNbllNVSS J103845+392736?ïüWþ)ø2?<mCù»?=@°…Ó?<mCù»?ïö¾|
Rà?R¤ºìغ?Rƒ	/¾?R¤ºìغ?ïn«¸ï¹û?‹çÄDÉû»?'*ˆåx\Œ?‹çÄDÉû»?ïõ&ïüŸ?Bv'ï"bo?U³Â¡8?Bv'ï"bo?ïþ)óæ¹?4«&&î?-`Å4dëf?4«&&î?ïÙ0æÛIp?uШ@|Ð?sgŒ‹Ô?uШ@|Ð?ïŽ_¯›—(?	¿·ß?Œh5ê?	¿·ß?ïÒlïl‰ì?lXÃ`Ëpy?vɈLz¹þ?lXÃ`ËpyAGN4FGL J1038.8-5312?áOha×û@ž!S6Þ¹À8à@
²
ªÀ;<ý7Σg@j ñ@¿,0	³?³Åé?ˆâ?ÂMŒ¥ÀC}@¾ó
N7›@VÌ=…Ç€¿ÙXVñ?¿Üôï#¿èçóߋ@e¿ëfL€S¿ïý—¥£"¿à&OÀ1³×AGNfsrq3FGL J1038.9-5311MRC 1036-529?ïü¤¸…p?7+âQ|–??:Ú>×ÆB?7+âQ|–??ïàÒ=?xZßß?o÷-©Ê~ë?xZßß?ï^äƒð…?5`s®¦?"#oƒ¶ýY?5`s®¦?ïÿÊ<=ŒÂ>ñž?à\û>úáÙ|½"Q>ñž?à\û?ïö|r†+?Qpo*N±?S넙?Qpo*N±?î½ý¾ %~?°\R2?¤ $"I+?°\R2?î:l;V\?¡'M‰?¬^)8ÚþC?¡'M‰?ïÿdòüiü?.d{à–?a¨t®rû?.d{à–AGN4FGL J1039.2-2848?çУý(gÜ@9¹:'£À:Ý¢'vgÀ<5ZŠ[@ G5««@XE ›€ú?ǘÓv	F¦¿ƒXÄx{£?¹'FÀÙ¤w?åЏ"Ýó¿å›°å"?ïUG$¿ˆ¿çРa3÷~¿ãÃ?ñBοÝJSá)¿ËòEžÅ¨AGNbcuNVSS J103921-285009?ïúWw¾±	?Fê"Ñ@&L?F¢!½fë®?Fê"Ñ@&L?ïpÿŒñB?˜ö>·zõ?'à`$‰Ë?˜ö>·zõ?יּa釡?…¦þuÖ	Ñ?"ѧ‰
³±?…¦þuÖ	Ñ?ïi
\Ç£?z¦°ÃS¿¬?'Þ´l2ø?z¦°ÃS¿¬?ïñ—d?d°á©7¥?]ùãUÚ7þ?d°á©7¥?êÜ¡ˆOÝ?Èöù	Ûe?čyß®ÀŒ?Èöù	Ûe?ï­@ŸR†?…í~?˜h¹?"¯ØFé΄?…í~?˜h¹?ê.'T.^?³rÚ1ŠÁ?ÇG™º¯Fˆ?³rÚ1ŠÁAGN4FGL J1039.6+0535¿ìÀ²ß±@Iüj%™íÀ;(D9P"À<‹RË~îó@!È¿¡ëù?ÿ(¥ߙX?Ä‹ªà¿¿¬ÄŒü*S?élIŸ†B¥?ùð3§!lŒ¿êF~3⅜¿êIEßaô¿åÎ	Bžá¿ØYɟñ¢o¿ÚKXC
ñ¿À|•|ÔfõAGNbcuNVSS J103940+053608?ïþy´W?àOôrÅö?(n#ò#?àOôrÅö?ïí;€eâ?d:—ºI"?bĹ6¼?d:—ºI"?ïó >íY?`°¿ÓM›?YÿÀÕüË?`°¿ÓM›?ïîFø•†?Lô€êÛ¼@?a¹A>™?Lô€êÛ¼@?ïþfX4Ü?ÙÞ5»7©?'éMùܯ?ÙÞ5»7©?ïm¤ÚPª?•ñ¾C©?Œ$–ÂŒ?•ñ¾C©?ïøÈ"îí^?_§µÏLßM?Lßsà<Nª?_§µÏLßM?ïGAN=Ç?ŽdT@ޒS?—Ö8ðÝ.?ŽdT@ޒSAGN4FGL J1039.9+7326¿íK…æoœV@DF~RvŠÀ:ÕüÍE˜'À<Œ>õßÎ@€®É"¾@µý}nÁ?ÄHGAˆ
¦?¦ý&Ô!¢?Ǥõ'Î{ù@W¹‹Ò[­?ïÿý²Gæ¿è7Æ´{G¿ç7"DZ£¿âÿ¤àõx¾¿ÝÀ‡å</[¿ç<V]çAGNbcu3FGL J1039.5+7324GB6 J1039+7326?ïþþX
-+?N_EÞ¶µ? ƒ-‹(?N_EÞ¶µ?ï÷+tð9[?R)¨ù¬?Q©þ'
j?R)¨ù¬?ï÷¡r^ŸÑ?TÎ\%¼?P½†N?TÎ\%¼?ïûÊ"öþ?$ží6—È?@×Òä¤?$ží6—È?ïþÍÃlѺ?"%N—ûÀ·?##Íq5ŸÃ?"%N—ûÀ·?ïÞl2"c
?qÍ©ýþÀ?pÉæ£@—	?qÍ©ýþÀ?ïøó?/ô?Z´¢>òį?O¤2"Ώ§?Z´¢>òį?ïñ*÷Çĝ?KÁ‰‰Q?]ªïEwu?KÁ‰‰QAGN4FGL J1040.5+0617¿Ü'ÀÁÚ3@JK¼'cÀ8®ìúi¾
À;éOâ–b­@'gÍï@ߢºª‹Y?¡­&ê$¡u?–¬þG»wÝ?ò'b`Ght@ЀÁÜXÜ?ïš	`ÑÑï¿âsù+Ðhc¿åf®à¨¡Ê¿ãùÓá>ó¿ä` Áìt¿îv¼àE¥|AGNbll3FGL J1040.4+0615GB6 J1040+0617?ïþŸq7?H»}µ÷#?&ð{DÐ
?H»}µ÷#?ïö¦óÒÓ«?UAyý/Ë?R²!=?UAyý/Ë?ïîcupDŒ?nq›^LßÕ?aœŠÌ4"?nq›^LßÕ?ïý«oÀ?'ãÀoIw?2¤ˆîÆPæ?'ãÀoIw?ïþ²k*N?°'ù	ëã?$ÙMÀ›ì?°'ù	ëã?ïÒ
¬n'?v½^¦`ö?vöyË7™?v½^¦`ö?ïè4µá›?sýÇ'
Â?g€ËÄÍ?sýÇ'
Â?ïü̏R?3ß0¦2Ӗ?9›‡ÖÍì?3ß0¦2ӖAGN4FGL J1041.0+1342¿å¯
ß0@LcZ…‡"ÞÀ:åA—z©À<'šÎLÿ@ æã'áït?ùj;rœÕŽ?ÏSƒµ¬ ?Í2›ˆ²¼?þªYö›s?ÿT<xl·¿íO˜ß_vˆ¿ÖìaÝÀþ¿äCŒ?Å(ggÃ2Å¿çDÊ•Œo¿Ûdçî'CAGNbll3FGL J1040.8+13421RXS J104057.7+134216?ïüLmä?0Âk!þ+??ƒF'?0Âk!þ+?ïéðè¬?dc•%i?fýÒ0?dc•%i?ïÛúû×?b9-–æ´É?rzv›ï0Ž?b9-–æ´É?ïÆ'þ»v'?b»Ox˜€?|ì¿ÑN?b»Ox˜€?ïùå"£?A´w‡ÒúÈ?Iˆk<á	š?A´w‡ÒúÈ?ï¥èòÈ4?‹wKC©?†…Ã@4 ?‹wKC©?ï·üDM|?ƒýâw»™»?'9€ðLy?ƒýâw»™»?î؀Ç]¬?']+hßH˜?¢wó†¾ÙA?']+hßH˜AGN4FGL J1041.1-1201¿á¯ºö>>@CÖî<³åÀ:Û·ìj÷ÆÀ<'á>sÙ@l^iAâù@‹QzF<?•5[×l8¿•õ¦4݂R?ӔÍí^<Ì@}禺¿?ïþòNf•`¿æ°ï@ëÁ¿ãøɪÙ\þ¿ÞBÀÄÖ´¿å/{]™c>¿ÄZÍÖâû7AGNbcu3FGL J1040.9-1205NVSS J104108-120332?ïýôI_ç¿?%LÑêGj?0]³"'×?%LÑêGj?ïó"Çz}u?W9gTì?XöqbûF?W9gTì?ï÷•Ö&Ï?A㶸T@?QâÔapÒ3?A㶸T@?ïöË£×àý?4¢âu7?Rh¸Ÿôõ†?4¢âu7?ïý§ªBM?*Ö«sZx?2®ᮗ4?*Ö«sZx?ïÑ°+"åÕ?zœŽgs™
?w'êWß©`?zœŽgs™
?ïö‹OÝk‰?]Á¦Mé	G?Ré`¯Î#?]Á¦Mé	G?ïÖ Ý_
?`ϳ•õ´?tï'a«…n?`ϳ•õ´AGN4FGL J1041.3-6437?ë²£1ʏÀ¸"~–À:FU-XÿÀ;É'§
öc@æE'ƒ@U0 Y;Û?̉WW)Ýt?Í(˜zŠ¶@.QYŽç@Gì.'ãÃ?álÝÿ$7î¿ëz¥î;²^¿ÜN?=­Š'¿è©]&KÄ$¿èŒM€¼S¿ïÿøsCÄ{AGNbcuAT20G J104117-643103?ïì/B…-?e™ðsÉe?cн:::ó?e™ðsÉe?ïãQ–u¢Ä?wvƒÿ!]q?l®iq ½?wvƒÿ!]q?äáÊ?"X‡š¯is?‡†Îl³R?"X‡š¯is?ïÞ×ø`4¯?Qç\Ûü'G?p"۔TM?Qç\Ûü'G?ï¶P™
*?'@>+f»?'kÙ©g_?'@>+f»?ïT¬ƒgdN?¦-ßÿ]‰?•jo›ª|&?¦-ßÿ]‰?íù´CáN?¡À͎^j(?°7J^¼Ü'?¡À͎^j(?ï"ò$cüC?…nIô:°ó?›¡»l¡?¶?…nIô:°óAGN4FGL J1041.7+3902?œOrj;ï@NEž:WëÀ;&¹f¾zúÀ<í¬v0@ –$d
q?úµE\*£B?ÌEB;å?ÌHäu_þm@ˆô'@–Ó–•ƒ?í0G@0q¸¿á<Ybþä¿Üï|ÚÇm¿ÁvÀ{°¥¿åÎUÎh®?¿Ö² c¢¼®AGNbll3FGL J1041.8+3901B3 1038+392?ïýü"Xx?!^Xö‹°d?0î¨/iK?!^Xö‹°d?ïó®•v–­?WCB"@¨?X¢ÔüÕ&Û?WCB"@¨?ïìhÕ<Ä?SÌKv?c—*›`vi?SÌKv?ïß×_3'†?PÎÇD|!?pPZ
¥?PÎÇD|!?ïýÄ-ŽP?*+šœïü?1ޕrb@¡?*+šœïü?ï×Öâ¥Q?um³M|
?tx½d?um³M|
?ïã'N5[ñ?r[à¹U£?ln±™)¯?r[à¹U£?SÞ_­?u&YWøv?‹×«øx§?u&YWøvAGN4FGL J1041.9-0557¿ïTSaÚn)@F95" ¼8À:}ïunA&À<tރ®uÊ@ C?F'ß¼@y—=žÇ?µ]ÉòíÉ¿°Þ-mÉÝ?üTDZ±?ýƼT¯"½?ïþþ๿èL[B›Ûé¿ãÑ/"‡•¿àqýƔϿÜiµ©yŒ¿½¿¨L÷?AGNbll3FGL J1042.0-0557PMN J1042-0558?ïû8¹Qg?6Y$ۄJ?C³*	0?6Y$ۄJ?ïÚ$·x|?tFßœ›?rí¤6ï>?tFßœ›?ïíçBh?d?w¶E±?búÃn÷Ô?d?w¶E±?ャ·"½x?bi¼¬£‰?€"Ò)îéë?bi¼¬£‰?ïõÍ^ºm?P ›q`ùE?UØe)ÍöB?P ›q`ùE?ïûˬ«?ŸáSǜD?œà†…C5?ŸáSǜD?ïä,üH¡–?s,m3nžB?kÓ´žºa?s,m3nžB?íÔïœQý?›_uµÑÃ?±_…C1"?›_uµÑÃAGN4FGL J1042.1-4128¿ØZM˲@.Pð"aùðÀ:×Ûô‡ýÀ<u]9—@ Îvúmˆ?û38Vˆ¢Ñ?ÅÈqÞ¿"~?Ïm¿$˜'@È\$Ä?þÄ·ÕnݿՁ¤k.Í?ŽP:¿Õ¨#>ߏ¿ÀÃ*Œ›"U¿á¬!±€–¿èT5vÚQñAGNbll3FGL J1042.1-41261RXS J104204.1-412936?ïÝsT¥7¡?j/ŠËíd?qFU¼'wH?j/ŠËíd?îçÇÕA:ˆ?¢‰h·V?¡ƒ'®€~?¢‰h·V?ïÁ"ºϑ?wÚc¶ IŠ?6#d‹z?wÚc¶ IŠ?îÜÞ7ƒNÿ?b3úîõ?¢2†B?b3úîõ?ï¤×¶ñÕV?'ƒ?Í6àU?†ÊQIg?'ƒ?Í6àU?ê‡×§h±'?Æà¬ë'x6?Åà¡b]9¹?Æà¬ë'x6?ï!q·Ý?•,í¼	Õ?[ÑÃôºf?•,í¼	Õ?êv]̱@w?©¿¥Ù»?Æ&ˆÍ:þ%?©¿¥Ù»AGN4FGL J1042.9+0054¿îÀ+)¤i@HÄ$¢v·íÀ:½°}á­/À<qÈAíá@!º˜AÕ¸?ûÀ…`ýpÚ?ÄÍM¦&ð?­orÿ{ö›?étÀœ<â	@½±@Õ2¿ãЯgÏG¿Þå8Ô\ä¿Ý´	½#ã¿ÙyFÄܾ¿ÖÅl†;¿ÝÿePfËAGNbcuRBS 0895?ïý
ÝÁÅ:?X…ƒÊ;Ù8?7'\¬êá?X…ƒÊ;Ù8?ïó"­+û9?\çÜ{¡ ?Xö¦=]"?\çÜ{¡ ?ïæ!ÌÐË?z4WLÓ\?iÞ2úúï·?z4WLÓ\?ïø Ñ"¨?6=€ÈÇ?O|"Â{€?6=€ÈÇ?ïüxK»?2Ùܚ_?<=§Jüï,?2Ùܚ_?ïÏR¾òLA?{°c
µg?xV n̛·?{°c
µg?ïï,©èW~?tÉVPé¯`?`ÓV0e±á?tÉVPé¯`?ïßBÊø-Æ?aŠ^µC?p^šté?aŠ^µCAGN4FGL J1043.2+2408¿ÝD»»ÏÇ@NƒCc,CÀ9e"7ÉÀ<EÞ)ìb"@½×f"@_åÏÓ?¬6ÂZOy?ªÛ½ç'Ý?ú"Ô%†¢F@¬m™‹Ô¿Þh_ž¡¿àB1Ó·¢™¿åWøyùÁ"¿äÄÔævÁþ¿æ[¹™ê!q¿å÷]š
_AGNfsrq3FGL J1043.1+2407B2 1040+24A?ïþMjQ>?1ÆF⣑²?+.ɉŒ?1ÆF⣑²?ï÷L•Yîß?PÅRGí?QfÕ¤Aû?PÅRGí?ïõ¹óA‰?U®ÛïB?TŒ‡J^‹?U®ÛïB?ï÷v¤Õ•|?@›(zÁ·?Q¶ÈGç©?@›(zÁ·?ïü×ïj±?E-†+H¥?;'A¡py
?E-†+H¥?ïÚp¹H?sZÀ¾h/e?rÇ£t7?sZÀ¾h/e?ïê¬K¢ë¨?o «AÇ×?eS´ƒ÷ñ?o «AÇ×?ïåŽ^@ìÉ?^r̆ðÙ?jq¡ÚÔ?^r̆ðÙAGN4FGL J1043.6+0654¿ÙZ@G¾z@JÆБ}kfÀ;CT¸¾øÏÀ<¤lõÌ @ `Áïy&@#gÁLf?ÍBœGHéÔ?}ó0e7?²9Ž‰@?ÿižª%¿¹aǛ4¤L¿äPpZÛï¿éz¿8åz¿Ì¾MØü¿åb'q	¿¼öLWFŽAGNbllNVSS J104323+065307?ïý×yNž?$Ä&¡k8?1D6Zkñ•?$Ä&¡k8?ïôH >	·?W¥™žù]*?Wn¿ÐãÑW?W¥™žù]*?ïò{çY…?Ldè_-[?[1¯Qö?Ldè_-[?ïõGQ.j?9£"ÅA±Õ?Uq]ã"‹.?9£"ÅA±Õ?ïüÒc)?6Î%¾J(^?9oîùÇÝO?6Î%¾J(^?ïŝØst?‰ÑgÆu¶4?}1rŒ7"?‰ÑgÆu¶4?ïó«Ã_27?aà¸a7×Í?X¨y#_'?aà¸a7×Í?+õ¸?oj‹!ÑGñ?€_§D!ú?oj‹!ÑGñAGN4FGL J1044.6+8053¿ïîÞøüß@A`»ÛãÁÀ9hùi
	ÔÀ;¶˜–dZó@ÓÕ)½"@'pOô4?²Ìx±—'?˼¤¡4™@'ÁC+λ@Ö»$,/¿±@}sž2¿ä(>ãjž¿ê×ÑÍmÜ¿ío±"‹c¿ïý"¶
+¿ï¤ÀßXÀ‹AGNfsrq3FGL J1044.4+8058S5 1039+81?ïžÐëjq¹?'vÿ¤²?ˆKÅ/²e¼?'vÿ¤²?î×Vh
ý¼?¨©>GüR}?¢Š™ $@?¨©>GüR}?îÖ*Žy?•_YÜß!`?¢ŸY²]g?•_YÜß!`?îDKD³Œ?Œÿh—4?«»K³IA?Œÿh—4?çÀE®«?Æýœƒ-òW?Ðt£Ú©ô?Æýœƒ-òW?çŸíè²?ÎÇØS5(£?ÐÁü%ø.?ÎÇØS5(£?é–úxµ&?³}þ³Ì
?ɤ+g•?³}þ³Ì
?Üã4Ç»b?·Sœ§Üv?áŽeøœ"O?·Sœ§ÜvMIXED4FGL J1045.3+2751¿ï²eîFo%@O
ÈuO7vÀ;<îM®ßÀ<¾TbWãí@ ÉýˆnU?ý÷¿¿ž!?ÅùcX¿ß©?o"=Äb™H?¨ÎI¾SÑþ@þߨF°"¿ïXPŽÌÝ?ïø]¿xÑM¿æ	°Š`A¿Û9ä<Õô>¿ÙiÝ^•a§¿ØÀäa>yAGNbllNVSS J104516+275136?ïÿhLçܕ?"›sçÉ÷?öj¢…c?"›sçÉ÷?ï÷ÜCüóË?T9¤ÿž?PGx†vžl?T9¤ÿž?ïöå;ÐÝö?SôwU]êÁ?R5ˆÁ8Ó´?SôwU]êÁ?ïý^®(?""¢Šâ?7CGQ=?""¢Šâ?ïÿ@à}?x[¢¯ý?wøµÛ%B?x[¢¯ý?ïÛâ
ªK?}wŸ+þXZ?rù†Øæz?}wŸ+þXZ?ïð¬Û•½l?oô•"šib?^¦HÄ	?oô•"šib?ïõôóKUƒ?I«²˜¤#ä?Tåéú?I«²˜¤#äAGN4FGL J1045.8-2928¿éKS·¦ä @9éã%Ô¦À9ù=¾§pÀ<?
›dtõ@…|Þwïü@ý.^¸<?¹ýjúIݚ?¶™_·ö|?ú¥)ð"R@uÏCtžã?J¼¼´¿æl¸ N¿è	ò&ùi
¿ã!ý•Âu¿ïÿù_|è3?à
 ÒH7AGNfsrq3FGL J1045.7-2926PKS B1043-291?ïý#£7?=36yp¯t?7†ãþ§nN?=36yp¯t?ïõSÙñÎd?\TDמ­˜?UXLMݗÄ?\TDמ­˜?ïÜö̶¸Ÿ?sFGÒŠ™?q"™£CØB?sFGÒŠ™?ïÿiâ>E'?B¸OV7ÿ?üÖýÅ?B¸OV7ÿ?ïýøs:W?.³ÉóÑOU?0<id)6ß?.³ÉóÑOU?ïÕ\~c»Å?^uƒF:?uQÀº4a¹?^uƒF:?ïÏ1=\#d?~7ÞÖG?xgablmÿ?~7ÞÖG?ïþl§£È?£ñ&pì?)5ÊwÔP?£ñ&pìAGN4FGL J1045.9-2331?ߝN&v@>úÓØYÈÉÀ:ãHÇïî:À<'âÐDP'@ðëzŒãÿ?ÿ.˜I7w?ÚÏyº×?×¹ügÅ?ý)–·g	ú@isyIm?ïÿˆ@«Áº¿èÑ–8W¿ÔâÜʶ¿êáôÃIk¿ç2Àç¼<\¿ïÿõž}.)AGNbcu3FGL J1045.5-2335NVSS J104603-232855?ïüYǓõ7?BRçç,
?=1Á²mŽ‡?BRçç,
?ïð"@'Hª?]u°œ·|?^÷€¤ú–?]u°œ·|?ïŠ
²'ëû?"Zå-[¢Ò?}Si"ÕP?"Zå-[¢Ò?ïàS0÷¦?QøPÞ½®­?o¬ÐC©÷?QøPÞ½®­?ïý†3ò\?7JÙ+Š@ö?3Îaؖ]?7JÙ+Š@ö?ïÉ^nÜgÜ?}U%h¨b?{PȨy~?}U%h¨b?ïR×úŒ?äc·øcÛ?•¥ÉS4t?äc·øcÛ?ï–§Yö–?t€ú¤9Ø?ŠOV:°fK?t€ú¤9ØAGN4FGL J1046.0+5448¿ïAÇ~6ð5@Kǟfb5À;;u¨ùˆíÀ<ԆðI©—@#·&rZ@u砍©¡?ƝÁ¿@"…4õ?ˆõŸeÉÆ?ún5ZTà,?î'l^YR¿éŠ¼A9[@¿åäÌh"ÿ	¿è¤8>4îõ¿ÉúÙh<¿ïÿÿ&¦³AGNbcu7C 1043+5505?ïü€[dÄ?1ÿ£"8ރ?;ÿ-–Èã?1ÿ£"8ރ?ïò"ããzõ?aûìTQ?ZÖ7Еõñ?aûìTQ?ï×FÎÏ#?qB¡ÕC9?t\˜«ÒK?qB¡ÕC9?ïí»N—Š?LEGˆRÄ?bD±+üÉ?LEGˆRÄ?ïû¨ ´Å3?9ùzpO?A_}ƒ:ý}?9ùzpO?ïÇђ{ºƒ?‡ê8?|6á:`?‡ê8?ïºûKÛß?¹`Õ
?A->IT?¹`Õ
?ïtK"±…ý?"'žËÎÈ??'vf_¤c?"'žËÎÈ?AGN4FGL J1046.8-2534?í®ÜøF«¿@=Y¦?šIÃÀ: ⴕžÀ<hHí¯›d@!V%–c.?ù½)Î/£?Èpà'ÒU?ʈÈ%ž:@hæŽ>ò"@7]kT¿éD,[Ø¿éýºÀÛ§Ü?͇ìH=o¿Ó—dá6¿Éø–T?È¿é"VœoAGNbll3FGL J1046.9-2531NVSS J104651-253547?ïøh'?F 8ðÄN?O›µ˜•ë4?F 8ðÄN?ïï'|Æ-?`~tœÙmÜ?`nâ¼óBÝ?`~tœÙmÜ?ïß?!—Ä?ozh»{!Ò?p`o 06~?ozh»{!Ò?ïí"óø¾K?I<?'s®?b{BZüÑ?I<?'s®?ï焕ó¿!?d.QÌׄ?h{ióƒ®Â?d.QÌׄ?ïÅB±ÍºU?+~¼|%H?}^§8¿=[?+~¼|%H?ï²!¿Ð?ˆÊÔ1?ƒwH|Úh?ˆÊÔ1?ﲺ-t³?vÒ3…ë?ƒQt­¢J?vÒ3…ëAGN4FGL J1047.2-5517¿ïí¢µ}@+ $bµØÀ9Ÿj'E'À;]ûî"‡ê@u¤œ×è@'iߗª¬?Å­W¼w¯?§YÿáÞ=?ܕĢܹ@«ÙK=¿áÏ$Ã-è¿ç–¾¡¿å,¥3Ìá¿çŠü4µê¿ê$¼ãJ½"¿ïú
ÝÿzAGNbcuPMN J1047-5513?ïüGm
0?4šÕù:??¥Â"׉?4šÕù:?ïݽ@Es?"¾:"?q!_ÙÖáÔ?"¾:"?ïÑ8ÂÇÃ×?r'>üs½??wcž"À¼š?r'>üs½??ïýµË±ø>?+ŒeFˆR?2Q£,BJY?+ŒeFˆR?ïø"[Ö¯?KFü£F	?Oå²YƊ?KFü£F	?ï§OJý?©­c
û?œëú?©­c
û?ïóyC?"»Í	ÙS¶?œ}a'‡¥¨?"»Í	ÙS¶?ïõAÎè—?HÆï'ß#?Uñ|x,Qº?HÆï'ß#AGN4FGL J1047.7+7238¿î+qØàVl@Dþ<Q‡À9òOƒËÑûÀ<H‡Þ†2µ@¶;ÁÍ@UYΨo?¼grUx?½Y''b?üR¬9¯N@ÍÉæhE?ª)'þþUä?ï_]"Y
¸¿áµ¹À€Ž0¿âö'î½b¿æ?)@k*¿ãþ±·!jAGNbll3FGL J1047.6+7240GB6 J1047+7238?ïþù¨‡?},¨W(O?.@b%)?},¨W(O?ïö²Œ§?Qà)c¸?Rޚ‰<÷?Qà)c¸?ïò9kºï?c6ÇmäsU?[(ãÊ"w?c6ÇmäsU?ïô\ýË·?C>Â\û_?WF|¯?C>Â\û_?ïü¹5ã‰?4¸ÇÇçà¶?:6PÃÔG¨?4¸ÇÇçà¶?ïÚûY…µë?sÈ¿{bÂ?r'Sèzâ?sÈ¿{bÂ?ïëíÆ0jE?r<vðK©?d9Ÿ{3g?r<vðK©?ïãû<V…?`Gñ(rJ*?líð
æ?`Gñ(rJ*AGN4FGL J1047.8-6216?ïí»QÐ,SÀ*~#ûÀ8ŸüuÀ;$ї6èÊ@nâP3@2²|¿n??°ú¥Î\
?²—ºÇ<@Nõ üÐ@ª;£!¿Ì<Õ"oß¿áùbW
-¿çOÒ:Ê×)¿æáÑv¹¿åö8Öá"Å¿ïÿþ½à ¿AGNbcu3FGL J1047.8-6216PMN J1047-6217?ïýÂ6'a?'PoÅ«KÞ?1îM»}?'PoÅ«KÞ?ïí.®-M?no|ó‰ÿ?bÑQž²¢õ?no|ó‰ÿ?ï‹'Œ§°?Œ ãptˆ?6õKè?Œ ãptˆ?ï÷ÙQÚ,?>B:ýQ¸®?QòM%Qè
?>B:ýQ¸®?ïû7{8ÒÒ??0}øÌóè?C"ƒ'¢??0}øÌóè?ïd,é~D?¦»7µ·?"zbÐ7n	?¦»7µ·?ï4-MYéÅ?•il;x¸?™zVO›]d?•il;x¸?ïÐJ"cW?iÒÞàK?wÚîÍÏhu?iÒÞàKAGN4FGL J1047.9+0055¿ßƶKÅ@I:ÀÛ'À:n©ö/yÀ<?µÚBV@@«6$)U@U`"¥?Ãá!¾Ð?©9½;	kd?à½2?î,™@'ûF²Â?ïÀRÀí ¿ç…Þz¿æÊjåQ¿ë°R®"½š¿Ã"úÉ4g¿ïÿ$m'MAGNbcuTXS 1045+011?ïþ'¬Ã?!oâ!°òV?'Õ2Ë€®?!oâ!°òV?ïô`±èè.?Yûb4œ­?W>œ+oôr?Yûb4œ­?ïî4ïI?Z¯ÄCàVL?aËòñ}8?Z¯ÄCàVL?ïü»x¢º;?)Š]ëÌí?:$8äOr5?)Š]ëÌí?ïþR¸Ý#?.'kM]T?*×$¸Œ3{?.'kM]T?ïÆݕÙô?#xN¸?|'5)}ö?#xN¸?ïÖáÒS°'?yH{TÄ,\?têr¯?yH{TÄ,\?ïèÐç
À³?_ïþö?g/Ääu\?_ïþöAGN4FGL J1047.9-3738?àÜ^ËÅïA@3*ýڋÒÀ:ÛCîlYÅÀ<ˆU|3WE@!"':ûSž?û9JÚåª?Æ*ñÛ¥Ø?¹ûOìýD?öâý¹÷@îA~5»¿ïýš?[à|?ïáäVVMê¿ÛÚ胿¼ŸXö;¿âd.þ›&¿Ým ßôq×AGNbcu3FGL J1047.8-3737GALEXASC J104756.99-373730.1?ïþe–æ>–?ˋ.5M¨?)¦"ï:´?ˋ.5M¨?ïéÁS‹²?gfUÓPßh?f>¬n΋ß?gfUÓPßh?ïóÀ؈þÓ?G9‹ð.?X~NoºÚ?G9‹ð.?ïíéœ*1q?Föáô7ï?bdi·?Föáô7ï?ïýh¨'b?)÷…i9Ò¶?4º¼R#|?)÷…i9Ò¶?ïŠÿÅ?H?•ó'Š ?@°>n?•ó'Š ?ïõêolkÛ?cË{/H‡v?T+ °õ¹Õ?cË{/H‡v?ﻐîéò?qˆ=àc+?9µ×'›?qˆ=àc+AGN4FGL J1048.0-1912¿îÔÛA.Él@Al½QðÀ:ùíp±CÀ<ƒCË0ëZ@†8sŽíï@ÞõfI
5?Ì}º•èŠ?À€È|)F?ñCâtÔ¾?û0£0œ*?ïÿì»"¿ÛÆDóO¿éÇ :ˆ¿ä/9ÿU5<¿ã¦ YžØ¿ïÿÿ" 5•AGNfsrqPKS 1045-18?ïüIŤm?7ÆdWÆá›?=±Ñ™ž?7ÆdWÆá›?ï´C¡jsf?Ž'"mBlš?'ï¯Z]?Ž'"mBlš?ï³T©ƒ$@?~·çë†I?ƒ*Õ£Vx?~·çë†I?ﵝÕt3?fL‰à"á?'˜¾Û!@?fL‰à"á?ïòŒ`ºÄ¦?c®RzT'ž?Zç>‡·a?c®RzT'ž?û>`t?¬~Õp‹é?¦THª\Ã?¬~Õp‹é?îùå'rÆØ?•ÓI•T£a? a­…cö'?•ÓI•T£a?ínǧä? ¶1q±?´YÁÊæ? ¶1q±AGN4FGL J1048.4+7143¿íûqºFQ7@E$	_$RÆÀ7"
ƒÁÀ;4òtý@/öU²9#@ ;>šo'?ÈîN…QÂ?µÂ¡"~–@&0¼Y¸:@!áªqKµ¿ïÿÚáb†¿ê[y£Z¼?ïî.¡©¡?ۜ@]=Gß¿àLZK¥ñ¿É¢
cAïAGNFSRQ3FGL J1048.4+7144S5 1044+71?íaµ¢Â?ß?ÈÓ3ä^
ý?´òRè¤&?ÈÓ3ä^
ý?ïßçAŠ?'
 úNvÄ?ppÌ|ã?'
 úNvÄ?íõë#Fx'?¡œË½ù¸?°P¦ç"	ð?¡œË½ù¸?ïÿ Ô`s? A5åðL?ý‹·? A5åðL?ï÷@˙"\?T0Blj™­?Q~hˆ!¡?T0Blj™­?ïZœm"\?²ˆÌ­6<?"¬rXDâ?²ˆÌ­6<?ïwÁ¶™?—)$@ÅûŸ?œÇÉ,Ú?—)$@ÅûŸ?ïü~™õZ?A&7–my?</¬ÀÈ?A&7–myAGN4FGL J1049.5+1548¿äÎXGa4ñ@MÉrGE8ïÀ9ï`sÞ.À<_þ99@I6ù;jº@$ù´Œ?¹äÖÙÀü	?¶‡ÑßÊð?úd§՟Ú@V'+áÛ'¿ä­òˆH8¿äJúú¿àc^Caÿ¿ãmó=yÞ¿ê´RbM}¿ßä«üƊAGNbll3FGL J1049.7+1548GB6 J1049+1548?ïúˆ†Ä!O?>ÿ%(ú­?EÝåÛßâÆ?>ÿ%(ú­?ïóNÚJö?Xùzl2?Ycñ×÷4ï?Xùzl2?ïØIÁ¯Û?vu¤xl?sÛt ‡ê±?vu¤xl?ïÐ6zÕ" ?b¿Y¡ ìs?w䃐øD?b¿Y¡ ìs?ïÝpµŽ†…?l8Lþ?qG¥&.Ù­?l8Lþ?ïÂ;͜¼ ?‹t|#ž?~â%ó?‹t|#ž?ïžz!ZÓ?ª4è@#?ˆawÐWW?ª4è@#?ï"ß †j?‰Ø-ª½kK?›¿Ä
§·?‰Ø-ª½kKAGN4FGL J1049.7+5011¿í¨§œš2¤@L¨6m
JÀ:îÂfA}yÀ<Õ? §?u@圧k@ÂeŽÐ?É7ôãí$Ü?ΏH\æ
?þJ†_¡P@é¶H¦âØ?îrò yI¿ãÊ\º³¿àd¸aý–¿æMzV[V¿ëoýV'n?Åb¸ÜÕÙfAGNbllNVSS J104857+500943?ïõ&Ka?P×KÕcBÉ?U³ã"?P×KÕcBÉ?ïôóÞoÈ¡?Vb¼ÜÁkÙ?VCWh}µ?Vb¼ÜÁkÙ?ﯠãԕ?z4ÙÁkƒ?"Ç‹êO?z4ÙÁkƒ?ïÛHÕJ¹{?T¥-k/
^?r[•YóVC?T¥-k/
^?ïð•"€LZ?\IDۑâœ?^Õ»b\
¬?\IDۑâœ?ïÓÎCøÛÒ?v…ÉŽ
?vÞ ší?v…ÉŽ
?ï'z¯ëâß?"iRI¬?›ªƒ¤ ?"iRI¬?ïelßãf(?|¨±[Jˆ?"Rdº¥?|¨±[JˆAGN4FGL J1049.8+1429¿²‰äÚÈ~ƒ@M'bS—WÀ9LwH5ù·À<2¾Ÿã_¶@q*EÎÁD@kÉÚª"?®žˆýÑ7Ò?²=ïN×Ôh@K¡F6E6@Ê
¥/$¿l{É:Ç¿ä«QݘL¿æ¯Õ`EK¿éœÀË6ʗ¿ð?ïþËÌÍAGNbcu3FGL J1049.8+1425MG1 J104945+1429?ïß?††J?®nX>®²?p`<ÚgœG?®nX>®²?ïö+ÁWO?UÔÓéåùý?S¨}×® ?UÔÓéåùý?ï˜$«tÒ)?‰ø{(ß*?‰öÕ"ËuÎ?‰ø{(ß*?ïûX$ü†?4ÆÚãš}r?BŸkŸgZl?4ÆÚãš}r?ïþ,­Kì×?+%ñ
I?-5'àû6•?+%ñ
I?ïÐÁ"ÖO>?€4š(š.é?wŸ='hÅ'?€4š(š.é?ï'äü:ðä?™{øw_?‹†Àà»?™{øw_?ïëÓ¸¤KÏ?Z'ØSì?d,G'z!?Z'ØSìAGN4FGL J1050.1+0432?ëþ{'Ï @J¨Ü]cˆfÀ9UóU͒À<,	óžÉ@Yø6zæ@uƒž?°‡ÇŸ'UR?³óÛÚ[×?þœÃk$;@£3ž¿Ý%#:—«ƒ¿åâ1ž½d¿æwKüWÔÓ¿ê\ÞCÖ¿çŽR"_¿ïþ‹ Z›AGNfsrq3FGL J1050.4+0435MG1 J105009+0433?ïþ÷\Bv?&_"U‰? Š?¦^(?&_"U‰?ïõWéSžÁ?YgKh´€?UP-'Hò?YgKh´€?ï©Ïá?]4Èû5@?`~nV0'?]4Èû5@?ïÿK{Ã4?0̊Qg?-	i±??0̊Qg?ïÿ…ÉØü†?€­²:?ŒµUJ´?€­²:?ïÑ+€%C?xçäѶw?wj?â_°f?xçäѶw?ïááà?k©Ý5Zà?nS ›?k©Ý5Zà?ïÿŒwG4?lÇsP¦?®vˆp5?lÇsP¦AGN4FGL J1051.2-6517¿Ê/1¯-2FÀ0¹~;oBÀ9l™ÝŒ7±À;·ÊX~F@"ýûÃÛ7@ÛØ{V¸s?´£è}ˆk?ªœ©!)£ñ?ô‹'æÎ×?ô
ôÀéú¿Ò.žÎ⧿Ö*èÁŸòú¿çм{Eñ|¿å¸/A8¿á¥Æ}þ2 ¿è"ó!uE§AGNbcu3FGL J1051.5-6517PKS 1049-650?ïô[qT?SDÛÊìí?WI`§j?SDÛÊìí?ï6ç%ú¡­?¡'Ã|^N?™#9̒[?¡'Ã|^N?ïzç˜?Šè[íÜx?¼ƒ#lˆî?Šè[íÜx?îÃÜi*™?‹y²¿¿[?£Â9j²?‹y²¿¿[?ïÂÞ–Èô?t¾ƒ3RÊ?~òӈ?t¾ƒ3RÊ?ê7ttWQ?É^Ç^s;?Ç"..¢»è?É^Ç^s;?ïšz
L?•?H•E!?Ÿl¾.R|?•?H•E!?æ	…™ÿ½\?¹°5M¥áb?ÓìôÌ…G?¹°5M¥ábAGN4FGL J1051.4-3139?½$ùšÇRK@8¡¢¤Û<À:žpÆ;¹À<OÚy]¹ï@ÿ·1Ô@LaÿÏ?Þ'_Tú-X?ïü«ë«µ@ BÛ@ í‹^B¿à‹ÛÀÛ|é¿æ(bÙ	¿ìÓ¤¢š¿è9ê™w5¿ÀÄbÛlwÍ¿àöÿ¦=ìËAGNfsrqPKS 1048-313?ïámnԅ9?ƒÕAšÊ´?n''½—?ƒÕAšÊ´?ïˆù)]W°?¦7¤³³^,?Áµž[@?¦7¤³³^,?îXúMÓ?žÐ$‰æã?ª~ ^®Í?žÐ$‰æã?&"W?'^Cæǐ?‹" /²X?'^Cæǐ?ïÚ{áo=?"_¼Ç?rÂVύy?"_¼Ç?êu·Öà:Ø?Ð<[ûÔL?Æ) ¤¢?Ð<[ûÔL?íü]	è®?¡"ôÖé÷¤?°Œ¡‹?¡"ôÖé÷¤?ãùpý¡´y?Ë`oçœ?Ø
¼—?Ë`oçœAGN4FGL J1051.4+3942¿èe±s½@OS?B5/À:Ò ùtÌÀ<'Ejm\$@!&Ö>°!?ù•¸~a.ï?Ä®j·ù?¼x`äÇ??úa…Æ}þ@B·¼Dif?ï÷"ÁpME¿è!œÓ	ý°?ƐöGo€A¿ä‰6?W-ä?±Ú, ‹À¿Ú"þPÅAGNbll3FGL J1051.4+3941RBS 0909?ïÿB'¦U?
ñ'ÅÈV?­¸þ.Í?
ñ'ÅÈV?ïøAƒ
¿?OÅM4Q1å?NùôûÂÌ?OÅM4Q1å?ïò˜©\?iè7ð²ß)?[òÏ,Xç?iè7ð²ß)?ïú~3À)"?2qOw—ç?F1Ýsâi?2qOw—ç?ïÿ€úÖ?Ӟïúì"?¯Ý>Ój?Ӟïúì"?ïØÇ¡Œ#²?wºFؗ‰\?sœ/FL¿?wºFؗ‰\?ïì7¯!sÌ?qó ˜'´?cÈQ$Ûô?qó ˜'´?ïñ1º¦ô:?Szÿ–sØi?]œŠéKä?Szÿ–sØiAGN4FGL J1051.6+2109?×1HîT@O
üçFÌÀ:Œ@O{hVÀ<Z)ôÆ@èåtc+?ýy*GÒ'?ÚÉLÅUŠ ?îâÁ*Øß@ã*!;¹ê@´ÏüØ`¿è³pÛ4n¿â.	È֞¿êqN õC¿ï£GÞ#¿ïLZUÕõ¿ënƒÁ@&·AGNfsrqOL 282?ïþˆ½Õ—?5?ôûôÿ?'~Æ¡Eù?5?ôûôÿ?ïô՝?W¸™˜¦­9?VTÅÔþŠ?W¸™˜¦­9?ïY‹Œ?'ÕûÞâ?ŸT·Ž´v?'ÕûÞâ?ïâ`O•?aVƒWSr?mŸåèÄ{x?aVƒWSr?ïýnŸ^ÄJ?Bp{Ä@¿?4‹ù8x?Bp{Ä@¿?ïÌàáà7ì?ˆm¤(¦?yõ
ó?ˆm¤(¦?ï­Œ7'×?•'˜C
?ŸêNwc7(?•'˜C
?ï¯p¤™—?~+'fò`"?"#ÏVٚT?~+'fò`"AGN4FGL J1051.9+0103?ÛfÄ|"œ@I¢pÁ3;—À:¨ÓÚGóÀ<zµ'»@ "~/Zá?ûÔ¶:º2?Éž–Xœy?ÊÁG3@nÙ8@ Þò¿%¿î^&@Üi"¿Â'Š^h@0¿ÔHÀc1þ€¿¶[Ø}Z¿ì\'Á3¤?ÀÅ`‡TG«AGNbll3FGL J1051.8+0105NVSS J105151+010312?ïõH ™?R
EæÆ?Un¿ø]!?R
EæÆ?ïðm‰×jò?\ZÓL¤?_$ì2íŒç?\ZÓL¤?ïL°v™©?"Kóo+Š?iñ,ÊÜ?"Kóo+Š?ïã#ä
Öô?U­1nê?lÜÄA?U­1nê?ïÓÿ'Χ¡?w¾þG$?v77˜«Z?w¾þG$?ïÁ²!¥Â?€"/¬DÞÙ?&ïN1Û?€"/¬DÞÙ?î³´ÝdA?™(õÐ0—?¤Ä²+s¼´?™(õÐ0—?ïˆ&Â.Â?}Ê«¶¯Ûw?öOt~Ï`?}Ê«¶¯ÛwAGN4FGL J1052.3+0818¿åáKŃàÓ@L.‹*kÀ;(Ï,"žÀ<€w˜½Ñ‡@éª{i,ê@‰$y\p?ÉÔ®ƒ
¶è?ŠÉ'"C
?¼"•£Àº@>%ühñ±?Á©p¨	¿éº¼"pdí¿Ù·áéÏ¿êÉÞÛÃ
¿Äpjá C'¿ïÜè‹+BAGNbcu3FGL J1052.0+08162MASX J10522451+0814095?ïþËñkÎÁ?ýMÞ6Ï?#@åÑDüG?ýMÞ6Ï?ïöv¥‰øù?Uˆg´A€?Sµ0Æ=ß?Uˆg´A€?ïål/Aû½?q˜›Âfµø?j"ÐÊbÛ1?q˜›Âfµø?ïþÓX"P;?«7äûjñ?"ÊwSS<–?«7äûjñ?ïþ¹µÝ‹Ñ?"JøY ?$džõ9"9?"JøY ?ïÓJe‡và?{Òahú?vZÍJ²ëú?{Òahú?ïæ)*NeÇ?sÐr$»8?iÖÕy@¡?sÐr$»8?ïù¾5Ái(?A^%Þ4 ë?I)[-Ò?A^%Þ4 ëAGN4FGL J1052.9-3743¿Ù/Ÿ°4Ò@3r§›ºÜ
À:ŒPx¾W¿À<|ÏÓèJ@ U*Ï?ÿI¦Wíþ?Áå'Ác?°JCp?7?óec>"º@,ŽTÁù4?íº|CG}¿ÀßsXd¿äµ¿Ý…*¡¿,ü¿Ð?›PÔ¿ë.
ß¼"šAGNbll3FGL J1052.8-3741PMN J1053-3743?ïûwsKt?TÅ×%&?C¶"ÉÕ?TÅ×%&?ïíR‰?cžåW	?b­êŗ_"?cžåW	?ïߒßì\?}ZRž1?p6óKfY?}ZRž1?ïñ»qä&Ž?A;}7 ¸?\‰[nÓU?A;}7 ¸?ïôã°Ê'?PpFTDE??V9Êҥ…?PpFTDE??ïÑ³L¯A?'òÖnÕë?ˆ‹",Ô/©?'òÖnÕë?ïܛk£3™?‡âC¦?q²JBSï?‡âC¦?ïÇÁÕÍÒ?k™Û¤§!ì?~<gêÄ?k™Û¤§!ìAGN4FGL J1053.7+4930¿ïÿä#«€Í@MEhÀ:´ñä´JÀ<m¶
éh@nˆcf?þ/}0­Fö?²ë¯α?žn"h¶?ìܲÞd#ì@.ø3
ò?' Wú?Ê
áÄÚ¿âd…†"¿Ýýc˜€À¿ä&@×`¥?º>¤@¼;AGNbll3FGL J1053.7+4929GB6 J1053+4930?ïþ€:ÅE;?`´÷A•?'üWěj	?`´÷A•?ïö™çi¨ˆ?T_¸§?RÌ13Q
?T_¸§?ïø9Piá?>0[°'Gå?O½T?>0[°'Gå?ïårá|Ñ?TàsÒÆ?jF÷2?TàsÒÆ?ïýðü	¯?.³'•Ì¤?7hw³ñüÙ?.³'•Ì¤?ïÜ©2W¯Ù?r'¡`ŽA?q«fÉÙ?†?r'¡`ŽA?ï÷÷J?cؒKæ?Qø:]%¢?cؒKæ?ïÃa`Ú?m	œ‹kú?~OO÷v²ü?m	œ‹kúAGN4FGL J1053.9+8628?çÑàAF@>0)à¤&À;7Žd²1@À<Œ†ÿc"@ =ºßd@W#"ú?ÆN­øvHÝ¿ˆGQ€Ù·Ê?Á<×xLm@(W$T9¿ïwWÂHå?í	ۂr¿ëx¤ Üš¿×ë'D"Wá¿Ï
W–꽤¿á#=Qš&‡AGNbcuWN B1046.1+8645?ïý6¥68?)¢4×F]?6JØ¢à…?)¢4×F]?ïõj®R@ó?XB@Ûª¼?U*£"¹i—?XB@Ûª¼?ïáè<aQ¡?ptò'½C?nÃ|RG1?ptò'½C?ïù€š¢¶¬?5xsP?Iý•XŽõ0?5xsP?ïìMÞQ§?c–ú¶r å?cô²ñN?c–ú¶r å?ïÏOŒ7äÑ?w؍'uÎ+?xX9Ò/Ÿl?w؍'uÎ+?ïÐÙÝè1?€ÅI±ˆþ^?w"FKC?€ÅI±ˆþ^?ïÑLŚBP?n™wʹºˆ?wYaøA?n™wʹºˆAGN4FGL J1054.2+3926¿ìp4c	Ç@O`ïܜM©À;Ê;"À<±ákÀB{@&a"ðh@h·¼šO¢?Ô	éã³ï?Ø*Ov`@ÇMœk2@J‰äDãŠ?ïì,CTéf?á£ÂýÁy¿â° ¬³R¿äiêIµU¸¿ïü`¾†¸ì¿é'kb#¶"AGNbcuCRATES J105433+392803?﹛‰«1i?vÉ[͉÷Â?™Š4åÐ?vÉ[͉÷Â?î¬*åJ¶Ì?¦åéôó'?¥=Q§ä÷@?¦åéôó'?2üÂ?'þ…í¸?¤F<Ó¯Ü?'þ…í¸?ì½¥#ÝÍ?—(ÎêÚ
?ºÖá—?—(ÎêÚ
?ï9ùU–à?"—Í?˜Ü Ó•Uø?"—Í?ê;÷"ÇçF?Æ£b!Ä\?Ç#tàbè?Æ£b!Ä\?ìŒïþ'Q2?¥OEëË?»˜€uvq?¥OEëË?㈃§óW.?¶å&ç0·i?Øîø°Q¤?¶å&ç0·iAGN4FGL J1054.5+2211¿ïf¹r|õ@O…" ä¶À9s€*]À<ò³ç#@,4XÍ@¼{ٕ2,?©?Ï£Á»¢?§S›2 ç?ü½CŠU@ÕàòŸ?ïû)×iß¿áón!EÊå¿â88 þ¿áI™;¥È|¿ä5D௭­¿äáü>ª_ºAGNbll3FGL J1054.5+221087GB 105148.6+222705?ïýø9àL? F–›S¼Õ?0?À6ÜZ¥? F–›S¼Õ?ïôÏ°VõZ?XÜ~ûÆzò?V`ŸL•ëž?XÜ~ûÆzò?ïõüÇnò…?cÜÁ:¶?Tp¹¦×Q?cÜÁ:¶?ïà|?ý­&?^‹A‹<i?oƒÀ/­²?^‹A‹<i?ïü°ë£Z@?.f˜H­"Z?:x£±°VN?.f˜H­"Z?ïڄäçÜÚ?t?Áöڞ?r½‡B#?t?Áöڞ?ï÷L«¢8?Z»‰u`ˆ?QgàÜõŸ	?Z»‰u`ˆ?﷜ã¿ÇE?t¾[|öÉ<?'ÇO¾ï?t¾[|öÉ<AGN4FGL J1055.5-0125¿ë¥0_)—d@I
ÅÁ?ÐÐÀ:G­§m—³À<OÏôŸy­@ >è{~ü_?ÿ‡ÚTtÌ?º›äbÈ¿ŸZ|Î1Ñ´?ä¥	Œ³@@"¯Ò–¿Ãòæ&¨¿ëù@€¿ÇK	ÿ\–¿Þ|_p#¿áb¡ N>§¿½@Y6}©AGNbllRX J1055.5-0126?ïûmø3¶n?6'hOÔ?BH#8*í?6'hOÔ?ïóEýȾ?['0âqŠ?Ytê/s2?['0âqŠ?ïñÑPaŽ³?jYrÞú?\]_ªÖ
?jYrÞú?ïïºaÄ?Fì#/[÷?`Ežc¥?Fì#/[÷?ïö•‡€Z?IàYGÍk?RÔñ6ùP?IàYGÍk?ïÆeìmý?"á…h©2?|ñM¨9ˆ?"á…h©2?ïòîûS{†?moˆ¹KŠ?Z"	tæ?moˆ¹KŠ?ïÀÊ9cgÈ?l(þÉ?šãb9×Ï?l(þÉAGN4FGL J1056.0+0253¿àT›
»xo@J£þ¬BêÀ;–(Ÿ~¶À<­¸6<Òï@#U´D•±-?÷UGZ1¥?Ð[j‰á•²?«™lÈ?Þ6B\Eü?ý¹U̐<?ë~·–ã?"(H7k?íjcì8¢ß?Ôìi ,°¸¿Ýê!;¹êr?Z9¡%BôAGNbllRX J1056.1+0252?ïþyè¤CÂ?À;Ëx€?(avAçØl?À;Ëx€?ïð$Ž?aÿ,ì¤?_˸Bþ?aÿ,ì¤?ïòt¿ÎS?J'vU¸É?[€£)[?J'vU¸É?ïàdO•b?`bÐ*_…
?o›±
GVT?`bÐ*_…
?ïþÒae? tMí?"ÙãaÕ? tMí?ïËUà"?€EDßw±?zUÄ#‹?€EDßw±?ïôOLÉ´?ddMò»m?Wafm¹i2?ddMò»m?ïÆ0lô
ó?um—…´´¤?|çÉzJZ?um—…´´¤AGN4FGL J1056.8+7012¿ä"ø| [ø@EôÚ<÷À9,azn['À:§9zu$@TdhµK&@Y£ÙŽ|?¿¯Ý'ãɾ?½*Œªü@	Ì΢âa@ÑD]'""?ؗ,¢z¿áø"»ìª¹¿è³Œdþ¿èžaŸ­.ø¿ìa‡"à¿ïý¥ýÖ.AGNfsrq3FGL J1058.1+7010S5 1053+70?ïátp"_?z3U`¦'?n‹9÷!$?z3U`¦'?ï÷`‹¶F?Qšc»]±?Q?ʋµ?Qšc»]±?ì˳+ÞLž?©}Â+;ˑ?¹¢f¡
›
?©}Â+;ˑ?ïüH?ðí?0&
ÿ^Ì??í¾¸ên?0&
ÿ^Ì?ïØ"PdÐ?xÍ|)Ü^?sù½åŒ÷?xÍ|)Ü^?ïÜ3º%ª?sðÑÛr¶?qæ#KÂï?sðÑÛr¶?í›	t"–?¤Æ}pv¾+?³'´Z•@Ò?¤Æ}pv¾+?ïâ‡.]
?cP£e†%Î?mxѩԚå?cP£e†%ÎAGN4FGL J1057.2+5510?é?'ì
Þ3@K"£½ßÊÀ;7='¨»À<á±¾SF@!-ÒK;é?óT5€ëM?ã9û¤P­?יG¤¯L^?û"üa'@˪ZÜð[¿íÂÎ{ùu¢?ä?°¿í#è§ô¦0?ÝWH…Ö¿Û'îM®ß¿êP
¤ž°ZAGNbcuSDSS J105707.47+551032.2?ïþC¿óJ?$"¢j¼J?+Ãüò-l¬?$"¢j¼J?ï÷¡0ßl?QM*î|³"?P½žsU‡¦?QM*î|³"?ïËÒ|ö1?tH¨)›*?zÁwØù\?tH¨)›*?ïüP@	Zr?*v¼ÃÛG	?=}ÿ¯­,?*v¼ÃÛG	?ïýÿy"¸×?4A	Î9?03iñ?4A	Î9?ïß×~V?pëc
ÿ?p@ôýÆ|?pëc
ÿ?ï¬$6?"ð¨-·òk?"ú6ØÓB?"ð¨-·òk?ïøÙ=—À?D·å97˜?L›9@R?D·å97˜AGN4FGL J1057.3-2341¿³1öÔ$ˆ@@ó.ZÀ9ã3cښìÀ<PÕ˨à@+³ß•ý-@SEø1Õ?»Ñá߃ˆ¶?ϙ‹Và·@r:½k/ú@Ü¥!âþ½¿ØHˆÚځ–¿Ú¬Cà‡¿äû…LXž¿é¼­?"¾¹¿é?#âqŽ¿ïÿס<%JAGNfsrq3FGL J1057.3-2341PKS B1054-234?ïö
B*>d?S//ÊFUg?Så|wö´?S//ÊFUg?ïíÆ)ùe?_þ&€W1J?b9ÕÔ%c>?_þ&€W1J?ïÍB[¢Æ?pQúþÌ>×?y^Ò'
Ã?pQúþÌ>×?ïÓÞÖSx?](zæW»?v"Öóãƒ?](zæW»?ï»Aˆt?"V	ãâʱ?/¸á§µ?"V	ãâʱ?諒Mö$?'Ò—ðqú?†¬…æ{£?'Ò—ðqú?î¾{Ñ»&»?˜,—ÿ¹?¤Bç½0P?˜,—ÿ¹?îèKHÜEn?Â'\"H?¡{Kv‡,?Â'\"HAGN4FGL J1057.8-2754¿á)'õ	@<•ŸÓo~=À9ùhG6‰À<BÃú–3´@ }'Ñ#I?ý"VÁ­´Ú?¸cfAR…´?®3Øþ?ö"æ™ýl¨@ WمÂÍ?ÑÀ&€ó/¿Þ=¡`¸Q–¿ß³þ4Måf¿ÒõJd¨ E¿æõ2F¤)@¿«ÀÀ9ÁAGNbll3FGL J1057.6-2754RX J1057.8-2753?ïþ€nx•?ÑïÙoAx?'þç~'Ç?ÑïÙoAx?ïô)4×£?ZØ=H~מ?W­–f·V²?ZØ=H~מ?ïóª;m?jÒ?mH@Ø?X«õW«›£?jÒ?mH@Ø?ïñ.tO?D'½c£•}?]£L•Ãk?D'½c£•}?ïüž2ýН?3ëÖò×?;jÙ-)?3ëÖò×?ïÏ":pú?yhÞt?Ç?xnâÊÆË?yhÞt?Ç?ïîqŠ»–?t¤Ñå÷$i?aŽâ¦¾É<?t¤Ñå÷$i?ïÔ£Žú§?`ADçE|?u®uÏ0'?`ADçE|AGN4FGL J1058.0+4305?à‡?ñ¨ò@O	V"À;Q4‡Ç	>À<ÔLR¾éµ@ÞÑrMû6@'¾´V?Áø­æ­ž‰¿«þym)N-?ê…¸Qì@	?Òñô¿ïãåÌÞÀ?ïÛ_W5¿é¦n£¿é~T>p©
¿bÜ­>‰u¿à¿Ýƒ(iAGNbllB3 1055+433?ïÿU)køæ?
sg{:æ?Z×'pQ'?
sg{:æ?ï÷Ù0fð?Pðcr?PMŸj¯?Pðcr?ïÚÄÈ­"‰?s<hõº'E?r›œ×#V?s<hõº'E?ïÿ4
$!?è9¿q"T?~º¢dÀB?è9¿q"T?ïû"}\y?E8"ÂÅÕV?A²4BžJ?E8"ÂÅÕV?ïÝøâ2]?vEer7b?qŽËwq­?vEer7b?ï¨"=ª¹?ˆÔ¥·ž¸?…÷7t‰µ?ˆÔ¥·ž¸?ïú‡ì{œ?EÏ·''ì?GÝ߇›RÂ?EÏ·''ìAGN4FGL J1058.4+0133?ïqãùD@JbëÝ3L^À7æR¯Ð=À;0;pïVe@À'D@…›"/Õ±?"rºÝŒ¾?¨¥ã»@'»=XP#@ÄaՈ¿ ªÆ©¿áw¾þX
¿ä'Þ^ð{S¿ã³'i#°¿åc(X䝤¿ç&ÆsxAGNBLL3FGL J1058.5+01334C +01.28?ïû"ÈÒc?9ÓÊðZe?AìÜäºîO?9ÓÊðZe?ïñ{Z"K&?`Míҋ'˜?]	K^c?`Míҋ'˜?ïÛ,Lâx?yJÛ÷?riÚ«ËÀ?yJÛ÷?ïúytF_?5{—à?¥Ï?F.€Bg?5{—à?¥Ï?ïý'²e\??3:'ß9+[?6Âm#.ÀÞ?3:'ß9+[?ïÅPðĉî?†~­ZË?}W‡|Üû?†~­ZË?ï㎾-?zj'[ ?lqïƒËo?zj'[ ?ïïX(Ì>?T"UJvO?`§Ø1AÒ?T"UJvOAGN4FGL J1058.5+8115¿å.7ö¼_@A_ d#–À9ÃÁ>#Q>À<¸Îé@'<ýâC'@÷¯~Þ,q?º °å¹±?Á¤Ÿ\&G?øQGñ0Yd@CäýÆö¿Þp*
ag¿æ5deÛ&¿æ€\a)惿äJ¯@ŸØM¿èæt¾˜×}¿ïóÓl#>ÉAGNfsrq3FGL J1058.4+8112S5 1053+81?ïýÝ.Þ?-œ' IÁ?7÷éXð?-œ' IÁ?ïöæw~øÀ?VQ÷‹S?R3ˆ¿/ï?VQ÷‹S?ïêWçónÍ?aºkR1Ç?e¨òJû?aºkR1Ç?ïý5;\]µ?#KÆød8?6V%P¿©Ó?#KÆød8?ïõ\_UÑ?PŽ'kb‡?UGûxNÚ?PŽ'kb‡?ïØÐ>x?w7;sÝi?s—ö
ÞCþ?w7;sÝi?ï ÍÅ<¬ü?‡Ö7ˆ4V?‡ÌŽ·³øû?‡Ö7ˆ4V?ï÷…µ-–3?C+6ܑ÷?Pô–Hú,?C+6ܑ÷AGN4FGL J1058.6+2817¿ë}ú"†4b@PCƒQX¸(À:%W¨]'À<vÄÀ§%@É{'G•Á@˜>{?´©8ÈôP?£×¡çñÁN?í²"\KZq@X¡C§¿ä|)±ª1—¿×ºÈ"W¿ä±õ桊)¿åñìa<°à¿â3͌æ-¿ä¥\{¬AGNbllGB6 J1058+2817?ïþŽèT{?¤,õ8z?'~úŸw±?¤,õ8z?ï÷'rXš?SjQ%¹,?Pûÿ
8?SjQ%¹,?ïó¾ÒýØ!?[¢û)÷Þ?X'Yž›MÜ?[¢û)÷Þ?ïýX@Ù?!¶Ð×Lá«?5=þ¤<®R?!¶Ð×Lá«?ïýOx°H?*ÝónÙ?5":Ï%Õ?*ÝónÙ?ïÚ`ÎnYò?{±~"?rϘ¼tnù?{±~"?ïôœG|s÷?b|Ò"?VÇpÇßA_?b|Ò"?ïø¸Ë*?>Xñh¬Q`?MŒÍò?>Xñh¬Q`AGN4FGL J1058.6-8003¿ìßµ~ÜnÀ2IêþæûLÀ8Òfàß©HÀ;ËûSÈÕ@<'UÓF@ö@×`¥?§Ã¾s?ÂÆ'De
@0¢_:ù@½r,mFT?áÀ½šTÕ¿Ðâî![Dt¿â֓ n¿ä‡âT1¿é|õSԓk¿ìð"rϏAGNbll3FGL J1058.5-8003PKS 1057-79?ïñ"†;y?]±ۦΛ?\Øó{ײ?]±ۦΛ?ïåe²·LÞ?ƒÃG5L?jšMapR	?ƒÃG5L?îU%`Y(ˆ? 'lr‡?ª­©öýۊ? 'lr‡?ïüα¤?1€k0"`??yGÁÌz?1€k0"`?ï›=_JØ?†ªM'tz?‰0¨7˜ÒÝ?†ªM'tz?ïµy‡±K?'ê†?¤Ð?'¡¸ÔÌ»O?'ê†?¤Ð?í©Øz™½ð?¥~ӏq"?²±<,{êú?¥~ӏq"?ï𹚯²ú?P~äAGšâ?^ŒËŽÊÈ?P~äAGšâAGN4FGL J1058.6+5627?×!{»7N @K7Y‰ßsÀ8+È5ŽWFÀ;‹ïXèÏb@B_ úa?ý¹"vD)û?šÀÜÿtê¹?§t®R¹5k@IÄ|œ2Ñ@§'ˆÛu¿Ð'¾^"¿Ür´þNúå¿ÝظG¿Ý…bÀi'¿âPÝèþÝ¿ÚbNAGNBLL3FGL J1058.6+5627TXS 1055+567?ïþÍ~´¢?5Þ¤âj?#(Ç¥??5Þ¤âj?ïöÉÀa¼?QÛƒ:.ê?Rlí7†Ã?QÛƒ:.ê?ïë±I8®?kL~4§?dN·
ª;E?kL~4§?ïý!¼'õ?&wJ9¥z«?6÷'Ð)?&wJ9¥z«?ïþžVâð?Qn Õm?&Ÿ"W?Qn Õm?ïàû!7Ìå?py:"ƒí?oÞÅskJ?py:"ƒí?ïìÜP"?iªL‰acU?c#ô'•Ä¥?iªL‰acU?ïûiÝ=â?6VƒZŽGH?BX‹êð?Ü?6VƒZŽGHAGN4FGL J1059.2-1134?ï1ϚÔÏr@EWçl‹C–À8*obŽj'À;ˆÅFƍî@0¿¿s@´ó\ƒŽ•?–Ä|=µ'?§*ò®~@
 "S.{>@#ùñÉ¿ÅžÚK:ö¿àˆbÚÀ«V¿âd["{L§¿á!Ä«–`¿å°pÀÝU[¿å7i=±;wAGNbll3FGL J1059.2-1133PKS B1056-113?ïþ$Üêbp?!iHÜ_ôç?-²0·²7?!iHÜ_ôç?ïóC8[]–?aú+;­T0?YyŽñNÔ%?aú+;­T0?ïðv²[SÛ?\ãJ1cd¨?_šÿ º;?\ãJ1cd¨?ïû '^Ñ`?2Iˆ?C}»(ŽC²?2Iˆ?ïþ	K5æõ?'£ãW?/kOÄ5fü?'£ãW?ïȗ¸»?S?~	üfAT?{´#dŸ?~	üfAT?ïâÐEcr§?u_p»u¡?m/º'pP×?u_p»u¡?ïõÍÁ?IÖuÆÂMî?UÅÈdì~?IÖuÆÂMîAGN4FGL J1059.5+2057?녗¨N@Oâ»ìª¸¦À:"'Gm|ÛÀ<o¼Õ±@‡Ñðøü@-›ymª(?Â;Ñ&ù"?®h˜Å´)¾?äsmµæz@	œ²êx"K¿ßÏÙ\'HC¿åF,iëV%¿å´üÌnÙ¿ä'zޢ߿ï\tÜJï?æusê³g¡AGNfsrq3FGL J1059.9+2056MG2 J105938+2057?ïý±%sÏR?(‰¼JÅ£¸?2vÖCz?(‰¼JÅ£¸?ïö%š)™?Si«Y#v–?S´ËOOm®?Si«Y#v–?ïêÛãߨ?bR¬lÿ`Š?e$áPp?bR¬lÿ`Š?ïú ÉÓb?4Q(:™åÐ?E|×Ö@?4Q(:™åÐ?ïýâ.û!?-ˆ'Fx6?0y¤$?-ˆ'Fx6?ïÖøâKÜo?tqMãø…?tƒŽÏÂô§?tqMãø…?ïÞ
M?nÊIVŽ?aE`ú;?nÊIVŽ?ïâ…K·l?_XDËÈ&0?mz´Ió¼ï?_XDËÈ&0AGN4FGL J1100.3+4020?ïàØˑA@OÈ<hfÀ:7|ˆçš®À<i÷_GŽ@ géAørî?û…tH§8¿?¾ÏtòÆ0¦?¼ìæÞýÝ@øSÜ &ç@I¾ð–*¤?ïsy³J¿âëÈæà>½à ¿(¿ÕJí#¯\¤¿ÙXI"ç«¿å#傦8AGNbll3FGL J1100.5+4020RX J1100.3+4019?ïü'ï!û?,"F"U]?;臙zrû?,"F"U]?ïïÂQÀ?^›í¡£'?`=®ä'çÓ?^›í¡£'?ïöUFÙXK?Zó´"H¸?SUrن?Zó´"H¸?ﶜˆ¦!?bÉji@»{?'XÝÍâ1Ê?bÉji@»{?ïøeOm¯?B¹	Ú»/?NjÂ
—¶…?B¹	Ú»/?ïËö³{?xörŽ9€?zy"¯á\a?xörŽ9€?ïõ÷ä†/?f½"ûê×?T6è¢%ç?f½"ûê×?îí—KûDô?‡ŸÀù?¡&‹<ÜÃ?‡ŸÀùAGN4FGL J1101.3+7017¿íñÖØ¥"E@Fÿ¼ä!À:CÃz=³ÀÀ:ìL>œóÁ@ÁÿiW@6
éh?·©׉>¿»iˆúe@G£áñø@]˜oVпÓÈ^˽X¿èéQgÑ q¿è]Áa^¿©¿é"'Ž¿á;Tiä ¿â\‹áõþÊAGNbcuGB6 J1102+7019?ïúÖ¤«µ??Nmû@(ãg?D¥nS"Œ?Nmû@(ãg?ïá6pv×ð?'¾Aà?nɏ†h_ö?'¾Aà?ï"äÒ¹1 ?•Kzü½ÿ?›£e®F?•Kzü½ÿ?ïîFœ>?[vÇlƓ×?a¹cäVh?[vÇlƓ×?ïð\U㮳?`ú5ºóÞ?_GTN æ?`ú5ºóÞ?î´l%Ã(?¶5g'?¤¹=£Ï}?¶5g'?ï¸ÙrD
?˜+jÂ	³?ŸˆäÎGâr?˜+jÂ	³?íŽØE¯jD?°/5Zp/?³‰=ѨÆâ?°/5Zp/AGN4FGL J1101.4+4108¿×"ð§`ö@O¹É>¢ÒþÀ:{V'Ý¶À<~CyÒSõ@ ·~"Z•x?ú#¶¾mŽ?ÂÅ Æt+?ÁȚx'·"@´ªFJ@‡¶HüÉ¿ð?ïÿþˆ0»Š¿Õ'îdw"÷¿Öh…ºêw-¿áÇq^-O¿ÌɄƒ\ì?AGNbll3FGL J1101.5+4106RX J1101.3+4108?ïý×>ÉG?(Ì1ˆŒ?1F	ÀÐ?(Ì1ˆŒ?ïòk%O#?XTîßé)?[)Ûà *â?XTîßé)?ïáåÊìð%?uϟû¶?n4Ó×?uϟû¶?ïÔxŒ·<?ZãqfJŸ?uúC¹¤b1?ZãqfJŸ?ïöÈXkHp?O=ùnZ?RoO.î€S?O=ùnZ?ïÒÖ%³e??u'ÐI©?v"íÿ̒?u'ÐI©?ïÓ h?~™˜ÈYd¼?voò¨®2?~™˜ÈYd¼?ïfîΡ°Œ?mƒ*N?""&(ZRŒ?mƒ*NAGN4FGL J1101.5+3904¿èWñWŠoI@P
j½ãû½À:ÊbhÀ;ÛHHn-Û@å	Yšü@·Káâ8?½š)¡äì©¿£âX¥2©ö?ä¤d~.Ú@¹ññIƒØ?ïþ;â¿ë-i$†È¿çWöÌz—v¿åé<oŽ¿ïþ%–c.¿âïÃÙßAGNbcuCRATES J110130+390434?ïô|¸§Æ?[ô»­?WŽþͳL?[ô»­?ïïL‹kOý?aævRRïL?`³t¡›`?aævRRïL?ï¯Æ<öç?ê×ÞÓ|k?"pÀæDW?ê×ÞÓ|k?ï•N0d¢?i*
ØÀ[?~µXù«§?i*
ØÀ[?ïËS³äÒ?ƒã›ÖjÇR?zV%÷™}¸?ƒã›ÖjÇR?ï¶G‡©A?"KÛ©<,Š?'náÛ?"KÛ©<,Š?îà—1µY¿?™²x	gb?¡öŒà^á?™²x	gb?íИ?Hã? W¬HÓ%?±K>áŸê? W¬HÓ%AGN4FGL J1102.0-6054?áYz)^?ž¿éæúàÜNJÀ7äè¼í[¹À:!_Ìqç@ñèÒ@Èÿ΁Ù?¶Hê¿üÚ²?Ñ XšËÈÁ@)Á¡ŸØ?ø_Y	¸&?écáPè¿Å§¼Ýk€'¿æ|fÃÊÆ¿ê"eҐ[¿êZ³R¨D¿ÕcŠAGNbcu3FGL J1101.9-60532MASS J11015838-6056516?¦4J=ô~Ù?¶Ô˜"©Z?\.v'?¶Ô˜"©Z?±gŒüDy?ª¼åäWê?íÓ`H±?ª¼åäWê?ΠºÑˆÚk?²£þ¨Î&$?èWÑKÉe?²£þ¨Î&$?•"?¸º?´E7.ÏÓ?ïS^-'?´E7.ÏÓ?o‡Ísû¢;?^=Çò?ïàx2ÁžE?^=Çò?]‹e=5?çEÊ;¯M?ïÁïE'?çEÊ;¯M?©DGƒÎá? c—Ì\[î?îk¾»£?ò? c—Ì\[î?$óè} t?°šµACÑ?ïþ°Ám6ÿ?°šµACÑPSR4FGL J1102.1+2249¿ïø»ºD£¸@P;$_ZÙjÀ:Ö0ã͚RÀ<y,;È-+@øãýëÓ£@
…É=?Ñ:~¯"®?Ïg	y{l?ýæª|¦D@B9_E0¿•CÐå5Nk¿åg©\…<¿ç›Ò>%Õ}¿ï=ò@¿ïՀ/eHY¿Ó0æ"ÀAGNfsrqCLASS J1102+2241?ïøšÉ¢ÿR?G'Õ'ñ&â?M"ØëGì?G'Õ'ñ&â?®å~?"ÈÁƉ?ŽQº^•tŒ?"ÈÁƉ?ïsKjr˶?…¶S¤òÝ?'–'³^WG?…¶S¤òÝ?ïMýyoê?|O±þq2é?–@]o4Í?|O±þq2é?ïõ6üûØ?W¶ç†''Ç?U"׍Î?W¶ç†''Ç?êìD´ê?ľ»	ç?ÄNí-ÀWž?ľ»	ç?íÌ%àLd?¡"B9Ëö?±žÐüaƒá?¡"B9Ëö?ènùÞ[s!?´žÅ^ù?ÎD†'3|?´žÅ^ùAGN4FGL J1102.6+5251¿îâˉ"J@L¦&€IRÀ:҈
%ðÀ<ʵ1¥"@V7éPf@¹eç»?˜ùJ"2ª?Ë*Pv%ã?úI·¿Ža@xh??ߺé
55¿âÿ^šj¿ê˜±¨ó¿æ>mhc¿ïÿØȃ'ð¿éd}Ãz=´AGNfsrq3FGL J1103.3+5239GB6 J1102+5249?ïúq"Ë?@Úü¦'–p?F9ôH?@Úü¦'–p?ï÷Xz{­\?Qƒ=–÷Cg?QO
Ély?Qƒ=–÷Cg?ïǤwv· ?os[·ù»t?|-Ä]a_ä?os[·ù»t?ïúú~zž?-¥¥dßuŸ?D"î?-¥¥dßuŸ?ïý	•É´?:±'¡ë·x?7·ÔgߋÁ?:±'¡ë·x?ïßÔ@ßn:?p°vNÅ?pßnœ·"?p°vNÅ?ïmªÌá‰a?&^äfòR?'J¦`_7ß?&^äfòR?ïî;Ftzô?OŒ¶UW/ã?aĹgÉ©?OŒ¶UW/ãAGN4FGL J1102.8-0148?Û~4R0é@I~þ£ßm¹À;¼pñÚ£OÀ<ÏQÕQ×@#E@tI	?÷c¬bäÒ?×(§¾öJu?Ì<ì™.:?õâíÖ1Ð]@J}ғ¶¿ïÿ^à54j¿ï'7*8¸®?ïøÞ6A?ÌõýR.Ì¿Ðó~}ÖÅ¿ã8ì£^iAGNbcuRX J1102.8-0148?ïýÖ¢ŽŠÈ?0s…õš‰8?1Jé€K«?0s…õš‰8?ïó+3	—®?[ÁWÃGRN?Y©™ÀÕ£ƒ?[ÁWÃGRN?ïèügçgO?^¡z¹dƒ?g˜ ×À¹?^¡z¹dƒ?ïøÙés1??0íÁÊ+ï?L˜ZØ	ó¯??0íÁÊ+ï?ïþÌR˜B? W(åæ?#:Ú~ÏùÌ? W(åæ?ïÃÑ
õ?"5µ@?~qy%™	?"5µ@?ïå`ï{oÚ?u‹§9^?jŸNö=û?u‹§9^?ïíTÈûi?`ú*w?b«8 þ^?`ú*wAGN4FGL J1102.9-5628?ètÐ*¿
0@
J¡¼}Ê0À:p.Ï÷#¸À<¨(÷@ »a•qA@:ëÄØí?Ç8§?¸Ÿ.ê#?íè*Át©ö?ÿ?®3Yž­?ïÿ!Í°"¿ìTç4¿³[H¿Ñ*™¿á‹	³Ýè~¿á%&_楿æÔù è­ÔAGNbcuAT20G J110315-562635?ï÷ñ&¯}m?FiÒÔ1hü?P²å½V?FiÒÔ1hü?ïÁºÈÆáY?•»÷4©?"›­½_i?•»÷4©?ïë÷¤*°ò?aH[I	Ø?d\	‰M?aH[I	Ø?ïˏ‹ùž?Y±s«J}q?z}8'uM'?Y±s«J}q?ïöt±¶N?N©µJN?SœQjbî?N©µJN?îZˆ±-δ?´vjÄÕß?ªWtëkFÁ?´vjÄÕß?ïÕ݀Še/?yÍñ"jPb?u?ÚiÐ?yÍñ"jPb?ïc½Ç2?†_
£®?"ˆ`öµµ?†_
£®AGN4FGL J1102.9+3014¿ÝõÓ4<j@P"
ú/§À:¢.›
³À<"îNý"@YÚ;JXê@!ï#8ê,?Äܸ¨'¦ã?ÀÖYh|?óQ+¡nz1@o%ý•—¿ÑW6]48—¿ê€O ý7¿é$¦©L•¿ìYƒßž
¿ï̚!ÿ¯"?âÉËûìu	AGNfsrqB2 1100+30B?ïÞX#ò<b?–gñbü¢?pÓîo³?–gñbü¢?ïÜË<Ôǘ?ø‹Âktî?qša'^d?ø‹Âktî?ï§MYؗ?€–Ö–†1
?†,©")q?€–Ö–†1
?ïÄæùÁ?mtü	²ýŠ?}Œƒ1Qtz?mtü	²ýŠ?ÔT€‹?™‹nzàZ™?ŽJà'	Y?™‹nzàZ™?î<ܝác?µLh:0e?¬26#¡œ}?µLh:0e?ï}ËÊKò?ŒÙzˆ›ë:?_fM‡À?ŒÙzˆ›ë:?ìzp}ª?®íçyʒ?¼/Ü|R­?®íçyʒAGN4FGL J1103.0+1157?îtÀ	¬t@N6#=òªÀ8ø€'Š×_À<uƒ9ÛÄ@ÌwȹlÉ@aGãÄ`?©6æ'xÀ?¸ÿXÿåAÒ@
@-¹€@çÀI‡¿Ø9ã{î¿á¾«6z'¿æt~¢Gh¿æfOõá™
¿ë aÉÁ¿Ý™åóíAGNfsrq3FGL J1103.1+1155TXS 1100+122?ïæ °ºœ?¦	=	ƒˆ÷?i_Ol_Þ?¦	=	ƒˆ÷?ï÷9|bB?S#:ÄVn'?Q3ûô?S#:ÄVn'?ïѲé!?wA1G#–º?wwqÅwë_?wA1G#–º?ïÿŒf'Y?¥Øü—e]?æŒw±ÍG?¥Øü—e]?ïü¸ÇKx?1ò	€ô?:9ǽyg?1ò	€ô?ïύz0š?{?ôòÉØ?x9C4æ?{?ôòÉØ?ïË° TðX?€5¸-kd?z'ï̘×Í?€5¸-kd?ïÿ¿û?'zRqmŽ?(öÛ­?'zRqmŽAGN4FGL J1103.6-2329¿ïÀ¶Íö²=@@‰ß¹8›RÀ9ï(ÝnۀÀ<![Ao6@ ø/']5?üNÞõÄ<Û?µ/Gì'Ü¿a*8'æÔ?«àÌVn@Y­í¹?íÕ»=®6_¿áâû{8†¿ãÌ?Ü¿Çïϛ´&
¿áÓìCÇ«?c…—ÓPAGNbll3FGL J1103.5-23291ES 1101-232?ïý{¦òü?%§ÙˆW4?4"Ç=-¾?%§ÙˆW4?ïôæ@x?W‹Ÿnç\¥?V3ò×ÀŸ,?W‹Ÿnç\¥?ï÷. ése?TäÇu	g?Q£¾VT"î?TäÇu	g?ïöNí41œ??KîÀmBÖ?Sb%Ö՗}??KîÀmBÖ?ïûg»Ñ?8ÕC%Òm?C§³ât?8ÕC%Òm?ïÑÑ


ô?~Db;Š$?wzìjë?~Db;Š$?ïð·Òâ?n'Ûò™Œò?^Zml9™?n'Ûò™Œò?ïêÉ1.B«?S÷IŽö?e6Îܼ?S÷IŽöAGN4FGL J1103.9-5357¿œhüŸ¡'"@š½†ìÀ83á
Ìq]À;Tª:э&@‰K+L‰ñ@-ÑyÚ·q?¢ß#í"¶?»p´yß@kK¯Ri@2("ž¿Ù"iʀA¿Õyœ^E¿ájè¬&d¿ám¬@eJÝ¿æœÜ¤Zé¿ê*ȀŒØ@AGNbll3FGL J1103.9-5357PKS 1101-536?ïù'!-ª¼?G
‰Zp?I»{;–¡E?G
‰Zp?ïÁЩ¦,?Ž{ªÄ"ìÉ?|—½
áÕ?Ž{ªÄ"ìÉ?ï°ÁDi¢—?‰8›ùzB?ƒÏ®óUÊ"?‰8›ùzB?ïþ(ceCë?Gó½—?-yÇUžçw?Gó½—?ïúññ¨?<æ©àî%»?D89ØaW?<æ©àî%»?í©£µQ[?¿÷pS>a?²²âVQs?¿÷pS>a?ï­få?Ø?Š¹^Èò©?"¦xMB?Š¹^Èò©?ïùó÷^è?=Ý´-F½?H0#O°Ð?=Ý´-F½AGN4FGL J1104.0+2611¿»B®æ²Ñú@PØ¾r–öÀ;-C8dÀ<Ì]°µ?@ ԁ÷çX?ý?óÖ&ã?Ò+ݾâ~e?Á,á	š³u?ïUa%´Åo@Æ̝|þ¿ä9&A³¿ïæ,Ÿ›;Z?ì°Âtºg¿Ñ´îV,\¿ì^ܙÉjB?É/-5A*AGNbcuSDSS J110357.29+261119.1?ïú;ËƬ?<éÃÃÂQK?Güo
	5?<éÃÃÂQK?ïôìr»?X"ú_áö?WÂ&çYšÃ?X"ú_áö?鍊QÌó±?€ª ªht?†Y+"¢KÔ?€ª ªht?ïÎfŸ"¦?i‰å&¡Þ™?xÌ° ßhš?i‰å&¡Þ™?ïø3dJF9?Gt·nÉ¢`?O2nøpf?Gt·nÉ¢`?ïÑ4pJ÷?€£á"´l?weÇðó]?€£á"´l?ï¸åò6=?ƒÓÍ Èê?ÆƒpÜ
Ö?ƒÓÍ Èê?ï€Û)Ëx?"Q¸nÅÕ=?É5"	?"Q¸nÅÕ=AGN4FGL J1104.0+0020¿ïÈÛµ ®@JiÝS¨À:ÕÀOæÈÀ<CHɝm@³k;p|@X¥}Ójv?Çg}'Hs¿'Âþ†r?Êd|ZÞs@Ga¶Scª¿ç¥ Jù"–¿æš¡¬bŸ¿à:â‰Ís¼¿îc!ãT¤?Æ8'}sHL¿ïÒìk΅4AGNbllNVSS J110356+002238?ïý°Ï#j?1"#–¹nl?2y†Æ"'{?1"#–¹nl?ïô¾ˆ¼Qª?ZEƒâ$—?V'î"œû+?ZEƒâ$—?ïÊÔ	W½?{ú">¼'k?z•û^‰Z?{ú">¼'k?ïþÙÇ(•m?rTƘ?"cŠ"Ê?rTƘ?ïùœIÞVž?Lb
Ñ2to?IŽ×'t›Ñ?Lb
Ñ2to?ïńsd-?•pk÷·?}=Æ`M9?•pk÷·?ïªZÑ ³C?†^nëÞ'?…iKª¿i?†^nëÞ'?ïò–Á*µ¿?X¡ô"-}?ZÒ}½ÒRX?X¡ô"-}AGN4FGL J1104.4+0730?èî4Tà÷@Lùfb4¨~À9ÎÕxlù(À<RæP+'~@ת«dÈ,@ϋÃîú?±ˆŒÖ脎¿ŠÚ6ÓâÑØ?Ø.‹-Æè@ñÑØzU?J´·,Q—¢¿æT²^âc¿æWúȈšn¿àzó†tù§¿ã{Ö[åÚ¿è-ç>"
¹AGNbll3FGL J1104.3+0730MG1 J110424+0730?ïþy°Î?@¥~Ü}?(dö…Ë	?@¥~Ü}?ïõ˜é‹G?Yÿ™¾°'ò?TÎ-e5X?Yÿ™¾°'ò?ïëP^¦Ý?xd»;­?d¯÷¦Ø'÷?xd»;­?ïýseÓC‰?!(Pˆ?4dÏ¥Iê=?!(Pˆ?ïþªV!Â?%´ÑºñU'?/µV‡'±:?%´ÑºñU'?ïÌBjÖ%?†-Êq0wu?yÞÊ««Y&?†-Êq0wu?ïëêÙʃ"?væós™?d&	l}?væós™?ïùíC‡5¶?7µn†­é?HJðû¶«'?7µn†­éAGN4FGL J1104.4+3812¿ç%ÅЕjq@PBIёXÀ5•v¡G
À:Óyq@'=ŒþU±?ûÄ£ÿYè?z}xf»?"×BÇzÓ[@º'®š²ž@Ô9ùËÞe¿Å¦²Ü¶¤Â¿Õ$è[Ÿ¹¿Ü‹Ù?Áa¿Ö¼/ʱ•¿ÞÙTšŒ¿ÓH__Œ«AGNBLL3FGL J1104.4+3812Mkn 421?î/ÇÀ•Ô5?º!>òŒ­?­ƒôêî¹?º!>òŒ­?ï÷£ûûÂ?Tžêç9?P¸õ>d?Tžêç9?ê†wº™?°8Ú¶u?Åæ!ãݜ?°8Ú¶u?ïÿ Ó/ù~?±ù´ˆ£ž?Ë)ÒwI?±ù´ˆ£ž?ïK—ÖJúÐ?š%¶¦xWÞ?–:Aù?š%¶¦xWÞ?ïÜ1÷tŽ?tŸÔ['Ï?qçrDy'?tŸÔ['Ï?ì~<ý‹R?¬šxSCm?¼¥q?¬šxSCm?ïÿÐP£?Ló¬mš>÷Ø͸à?Ló¬mšAGN4FGL J1104.9+5748¿è#ÉlßÁ
@K	pŸM8À;cpè hÀ<¿Pû›@Þs1s•@ÈPïܜ?ÃNwëC?NVq¬˜@	æ4á‰t¿í⯢št5?ïÚ==£#±¿í²•~æ¿Ò•!û'~¿ãÎCYñãÞ¿ïÿûÎBÓAGNbcu7C 1101+5808?ïÿ
¨Ej)?'±bì ?Jü··}ž?'±bì ?ïø>y§$¶?Pûˆì¾©?OPPœ?Pûˆì¾©?ï°ï[9ƒý?ƒúçnp?ƒÄ)9ÞÎ?ƒúçnp?ïýÄxp?â(Ìƛ"?1ßL%hÏÑ?â(Ìƛ"?ïýó׎r?@'BDìH'?0g'o·ê?@'BDìH'?ïÝíÔâÎt?rÃ¥ÑGE8?q	¬ÕU›?rÃ¥ÑGE8?ïpPöù­<?'b—ʘ‡N?'õá ÊX‡?'b—ʘ‡N?ïõÏ|i?L¯K÷"‡°?Tàb?ýš?L¯K÷"‡°AGN4FGL J1105.8+3944?î¨Cïª-¢@P0O"}ŠÀ;/øìÀ<"Ž7£@N´¾c(@מà*w£?««u+%¿¶ï«^"[?ôÏ|ªuŠ@ƒ+ÍcJ¨?ïöaD=¿æ6M½øô¿è;$,/3¿ãÓø:8àò¿Á')™¿ç¥0 Y;ÛAGNbllGB6 J1105+3946?ïýÀ ¢*?$"‰'DvŒ?1úü1ñ…?$"‰'DvŒ?ïõÿrÞ¼0?SžÞs=?T—½ï¸?SžÞs=?ïïªU\0‹?n¬¹R?`UªÈë<·?n¬¹R?ïù̼©
?5'¦pÞ¦	?HÍ®S?5'¦pÞ¦	?ïûäû Ry?7d‰Ÿ¾—×?@l¦×ò>?7d‰Ÿ¾—×?ï×)K€?t':E8S?tkxQPü±?t':E8S?ï軽}Eó?uJœu?gDBo|<Ï?uJœu?ïÂA<¥µ?t·-y®?~ßaÎsåY?t·-y®AGN4FGL J1105.8-0731?ÚB6LS{ä@Gx ě¥ãÀ:ž'jöîßÀ<yÿ ^°@™½€Ô@ˆR]S?¿óâæ>¸Í?qbÿ»Ô°?³|{P®CJ?þ!/}F&Ö?ï¦rÅð9¹¿ä†ÿ=T<¿äûà^d¿Ù¦-¼%à¿áE}Ð:k¿èppçɨAGNbcuNVSS J110547-073235?ïúö2÷¤?5ÒLÍÇ©?D'4³+†?5ÒLÍÇ©?ïïé5Òäƒ?\›•öã}ê?`Ê_õ´ÿ?\›•öã}ê?ïòŸà–¿?Wˆ­éÕÂ¥?[ÔÀYaž?Wˆ­éÕÂ¥?ïäR1ž‰?Pšâœ¨Nâ?k­àÝ¿T?Pšâœ¨Nâ?ïóÊ)ÚD?N ß"ú?Xk¬Áª‡æ?N ß"ú?ïÌò¢Â?xsÑ
*š˜?y÷u{¯ß8?xsÑ
*š˜?ïöaB‡†i?\-§¡ñ?S={a¦]T?\-§¡ñ?ï‡3ڑË3?v¤g¸©ßÍ?Ž3	MÎÃ\?v¤g¸©ßÍAGN4FGL J1106.0+2813¿ïÂ}ØÆ@P«hœ¡‹ÖÀ9TWuÇ,À<NÄ3¡<@ýñò¡Æ@®iŸÖÊ}?«ï°GÀç?²‰»ÀŠõ@¤m'ºZ@f,I	3Z?äQXí×ßP¿â	û+"é¿å±€`b–M¿åâ£cF÷5¿èۅ⭉¼¿æðÎ3Õ¢AGNfsrq3FGL J1105.9+2814MG2 J110606+2812?ïþï@ü?MW1¤A°?.ΐ‡ÿ=º?MW1¤A°?ï÷Æ鑇/?PûúT÷W?Pr,˜9r=?PûúT÷W?ïîipP?L.#¯dE,?aî–h
7Ò?L.#¯dE,?ïû¢oߕ?3‹´'?Cýw?"ø?3‹´'?ïý¼uf´?*"Íã·£?7b»;4X?*"Íã·£?ïØ¡Û÷&?yªÚ8ÚÖ?s¯õN·Ð?yªÚ8ÚÖ?ïÚ?í^pV?u†ªyyµ?rà	L¨L×?u†ªyyµ?ïô)'Ò¾?KøKj?Wϭٕө?KøKjAGN4FGL J1106.2-1048¿¤á¤+9@F$ÐgŒTÀ:÷!' ÿTÀ<U1Š¼‡@ôðVÝØ@Cœzª?Â\x¦Ú'¿–¬fzÞB–?Ò»-½þR×@¦`s^™¿ïÒ͖ h?êÜøɪÙ]¿âyJ]d¿ç#•Þùö¿Ô±JG
¿æk¿Á¡u†AGNbcuPMN J1106-1048?ïýÅã?*u²8‹?7ñÙ[,tÉ?*u²8‹?ïò%/uŸ¦?_ò«Áà¸?[µ –OŸ?_ò«Áà¸?ïç–v=bÑ?f—¢ 2ÍÎ?hi‰•BWv?f—¢ 2ÍÎ?ïø
WMç?9åÂiVÍ?OÊ¢15®?9åÂiVÍ?ïôD?Êñ*?P*¿\,$?Ww€‹êÞ?P*¿\,$?ïÉ[=Þï?{ž3I¿úÊ?{R@['(?{ž3I¿úÊ?ïÙ¤ó ?zԏ0®wc?s-ñ!bGÀ?zԏ0®wc?ïÔ}ŽÝ9=?j´õؙ;?uÁ8¦°õ~?j´õؙ;AGN4FGL J1106.5-3646¿âEn¼§@5€"xÐÌ6À9ÉÌIN†À<D¨£!ؘ@IV
M·@ƒŽ)ùΎ?´}íì'Ô?³íóŽ¶@VÆž@
ï6ŽÝS?ïÿÐß´¿Þg=;tË.¿äø~+	Ë¿ÒÞc£",¿êJÔø³¿Ô¬Âû<ÍAGNbll3FGL J1106.4-3643PMN J1106-3647?ïüŸîrcö?0סA"›?;Šmšu×?0סA"›?ïïpÆf¬1?baYAPá|?`9T›žé?baYAPá|?ïãؘ´\?rTéƒo?l'h!Æ!?rTéƒo?ïì£zÕ‰?JŠÂÜ¥>?c\…J'ß1?JŠÂÜ¥>?ïùT°–Ã?Ey^àÂn?J­@Žw?Ey^àÂn?ïºÀP»>?"O<›Â3Ü?Oëú1Xk?"O<›Â3Ü?ï­PHþݧ?ˆKh¨Þ.?"«íÀH–-?ˆKh¨Þ.?ïÂm%¥ß?i5dÅS¨?~Ém0Û ?i5dÅS¨AGN4FGL J1107.0-4449?‰˜7ÍTe@,hÆ÷ µîÀ9!—q¡-À;ã¬ÍSŠ@kêÈ5cd@lŒPû?²
	È««?Ñnîàå@¦ýòÆ@D€t¯_¿ÌN
$=H¿ã•è41_ô¿éÙ(?º*3¿ë"` SÈ¿ëÂbæ%z¿ïÿ£NNA¬AGNfsrq3FGL J1107.4-4447PKS 1104-445?ïl£wî?ªWG¦½—?'k'Ÿ"E?ªWG¦½—?ïȘ粬?u·Óår?{³òóiz?u·Óår?íšÂÐöÆ?£í-Üb?³)遐Î?£í-Üb?ïÞýNIäû?WcT©F« ?pXõÚv$?WcT©F« ?î¸uQ槔?¢q‰d€"É?¤xªå"¶?¢q‰d€"É?î,Ø?
›©?´žF½Ù³É?­2|¡Èg?´žF½Ù³É?í
š=z×?§'jAÜ&.?·¯S+îgÊ?§'jAÜ&.?î¦7ªÄÂÆ?'ôýŠ³6t?¥œ…S³Ó¤?'ôýŠ³6tAGN4FGL J1107.6+0222¿Þ? î'\@KvX£/D'À9ÙÒø_øŽÀ<?x½€ÿo@¹Ggž@À¥ýU*Õ?´ÀÿÚÁ,¿Œ:Úzm?ØuzÖµ?ü]JÑ_ƒž?ï••9¹¿â$çî'C¿ä90m†X¿ÚÃ*¢8¿ÚA	8x¿ç0ãݵ}PAGNbll3FGL J1107.5+0223NVSS J110735+022225?ï÷®×樸?DecŽÑæƒ?P¢P¹_>u?DecŽÑæƒ?ïì"ü?d˜ÔT	r?cììXû¶?d˜ÔT	r?ïßå!¬´?qÖËMx³5?p
8z(eÔ?qÖËMx³5?ï¹âîæìÍ?j¡"kª^?‡D;ž¶?j¡"kª^?ïéSµ×	^?]""‰{??f¬J$×ì?]""‰{??ï¼ ¨›Y?€Â1&_XŠ?€ÿ×â7Á°?€Â1&_XŠ?ïÇù
dÕ9?'v½8ª?|zäBÏN?'v½8ª?îêè‡øî?y'üKÕ?¡Q~ê&?y'üKÕAGN4FGL J1107.7-3042?².ØãÀ@;R¤ À:Õó‡K¹<À<u¿î¼@v™!N¯;@éœzõj?Âð¼@7¨Ž?e1Àz*©Ò?Ÿ˜<æÿí¥@»^ÃYÜj¿ÛMšÝ¼^@¿ÝǟÑÁÿ¿æ}‡ ¿ìTÃ;S"%?Μ­ 6Á³¿ïÿÉy[5±AGNfsrqPKS 1105-304?ïýÿY^bƒ?&Ly>Ì6ý?06¸¡©š?&Ly>Ì6ý?ïõ‹›1Ò¿?VÙÈ}n«?TèÉД'ª?VÙÈ}n«?ïä/ܲ?h÷D§õ1?kÐîáôÎ?h÷D§õ1?ïÿ}lEC?r"¸íž¾?Runüõ­?r"¸íž¾?ïúfhó<+?Iÿõ	v?Ff\½?Iÿõ	v?ïÖiŠƒk?vÌ·kûz?tË:ë:¬?vÌ·kûz?ï©{æo$?†‡qSl?…¡n…Îô?†‡qSl?ïûٞÜ?<TÒ¬>¶?@™…;<z?<TÒ¬>¶AGN4FGL J1107.8+1501¿Ò_¬wd@O‡EŒÒ
úÀ9À]''N#À<<Ò@ª;@+ÍcJ¨?ýÄÔ`?ù?¶šCžÌo–?µÀf#z@By<,9@0™)^"?ïÆ-vZÐ0¿àÿø¾m8"¿Ýw¥Þ¡`¿Õ7Í¡³ï[¿áp #‹öC¿åšíV°AGNbll3FGL J1107.8+1502RX J1107.7+1502?ïúHp‡&¥?:¿;.Ô?FÞ=XNÔî?:¿;.Ô?ïØß•—¾?w?@‰dH?s~ŲA%?w?@‰dH?ïá!×QqH?prôÚ1M?nÞ(¤ïÐ?prôÚ1M?ïMò¼f?x£jÑÓí?–A¨}s??x£jÑÓí?ïìæšÿZ?V_›«"?cdÛÄÝÐ?V_›«"?ï…ÛÜ+±×?|ƐwÐÕ?Ž‰	Ñú0?|ƐwÐÕ?ïĚƌ¹.?'DOçÂô?}²œÛO"æ?'DOçÂô?í[L+ý‰Ù?œéb±Zhr?µ%žŸ7Ê9?œéb±ZhrAGN4FGL J1108.7-1844?·êçhûQ@BçÁß3ÞÀ:Ò
(ÝnÛÀ<kDTæ³@¾òÖ§l?ÿž\\!i?ÎÏÅåýËG?ÂU½ ÝE@?ò®²Jj‡]@Z©è"8?Ò ~:Bœ¿ãOäÿÉy[¿â˜¶DË¿ç¡â"o¿Áô×ÃJíå¿éø@~AGNbcuNVSS J110845-184505?ïý?¬¤?2 ùÕÂ
?7öëüŠ?2 ùÕÂ
?ïó^&¨?\
Rs¨3ß?YïD	.þÌ?\
Rs¨3ß?ïç Gjš?n¸¨XÉ?h߸†G˜ø?n¸¨XÉ?ïö;BÖ?;|k–n?S׉…SÏ?;|k–n?ï÷´´ýù?I«á<<é?P––	6¦?I«á<<é?ïÅÁåp»?ÃF­`»J?}qï'?ÃF­`»J?ïÕ,ëyï?wî»ЀÜ?uiŠK¬y?wî»ЀÜ?ïÉÍ®?pÓ¥F‡Œ?~;p~£5-?pÓ¥F‡ŒAGN4FGL J1109.3+2411?äø±ÆÐÎ(@P¶'Ìö¾8À:?9ÉOiËÀ<g¨"1 Œ@ 
¸÷'Øã?ýwM©Öþ?¼çýÀ4¸ï?¥uø)Çύ?닫à.@[¨ý?ëÄ'¬í3u¿Û懞olI¿àÔN¡MÿÖח`Ú5k¿áüÄʟ̿̂ XÐ{®AGNbll3FGL J1109.4+24111ES 1106+244?ïü*yêìa?.8u€œÝ?>¬/œUZ?.8u€œÝ?ïôÊê?
?U½ÔñV?VkßÃ
Í?U½ÔñV?ïòC"Â¥Š?XL—"n^?[xö›±+œ?XL—"n^?ïÛ‰êqp?W
^­Y·?r~»W¬?W
^­Y·?ï÷cT@Ҍ?BPïrj=?Q9V÷ª9Y?BPïrj=?ïӈ"Iß®?vähšÓ?v;µüh·?vähšÓ?ïõÐidr›?båjxOå?T_-pÔ9
?båjxOå?ïŽ~[XHõ?u…Š;ØFF?Œ`i7¬2±?u…Š;ØFFAGN4FGL J1109.6+3735¿ÅVIZ3t™@PŒ°á´»^À:¶'néšÀ<…ý	«zm@ óÿ'¥?ù,Ø:¿¯?ÐKs›Ù?ÈTµyt
>?ø7ó÷´$@	àŸµg€m¿â¢X_g™—¿ì곝PÞ?¿ÑO7
XH–¿ÓØLÝ©=ü¿ßŒDý
,T¿àcŠØûAGNbll3FGL J1109.6+3734NVSS J110938+373609?ïþà‡"L?ºñ ]®ª?!þ§WZ\
?ºñ ]®ª?ï÷±$OÀˆ?Q$ۂ£X?P¶õK!a?Q$ۂ£X?ïñÀ‹I†?QC'´™Zö?\áAbó®?QC'´™Zö?ïûV¥~?.qäA<w?C«Î¶tä?.qäA<w?ïÿH…³fR?ÎiåE?ïAj"ãy?ÎiåE?ïß¹$?s¦ƒ3éøë?p#|òÇð³?s¦ƒ3éøë?ïñey+1?dÍì0}"?]5×iLÿ?dÍì0}"?ïô_vná?FéÜêéU"?W@áR[
¸?FéÜêéU"AGN4FGL J1109.7-4814¿ïÓ¿Q±oñ@&êþæûLÀ:³þËLš
À<ËRyI˜@øS*I¦@|š»É.?Êh'äÄeJ?Á	pT§?óøÜP'`@í}ÃOJ–¿çÕ\¾Fø¿àPVXÍ÷¿ëbâ¸Ç\K¿Ý©àc­y¿åzэ%íпïÿÊPʇAGNbcu3FGL J1109.4-4815PMN J1109-4815?ïþl±GúÚ?#o¿Ò.m?)4è6†ö?#o¿Ò.m?ïétUge•?p´>¶%?f‹ªÙ3Ì?p´>¶%?ïã`/8R?os½ÃÃ[?lŸôàõØ?os½ÃÃ[?ïûñÉ'r?'Hou"'=?@8Ùý˜4Õ?'Hou"'=?ïøj'ùtÿ?S]nÿâÆ?NU´î`¯n?S]nÿâÆ?ïUÀؼˆ÷?ŸwŠuZ?•GääÿE0?ŸwŠuZ?ïfe\3Ì?''N"'í?"3^ïR}?''N"'í?ïÝO3ø]¨?câ[F¦P?qXf#m"ç?câ[F¦PAGN4FGL J1110.2+7135¿½¹^+À‰Y@E°U2a|À:m«|ðìÀ<­ú4ää@ ÛN?üºØÿ
6»?ºŸJžê	?ÀÄø(e¥@Ÿãåî@æÏ¥DG®¿îfºI<‰ô?ïœàÁ q:¿È¶ÅúJ´Y¿ÚI›)'Ÿ¿ç*J+Ú¿¿=ç—({AGNbll3FGL J1110.0+7134RX J1110.5+7133?ïþ|
±]?#"uLo@N?/BfX3°?#"uLo@N?ïêêãŸ]d?f½ênJÅ?ežÛ¸?f½ênJÅ?ïñ߀ë?[—1í‡?]ÄA¸…
Í?[—1í‡?!':Ä?mùû-".æ?‹Ÿ÷'"zõ?mùû-".æ?ïñˆ˜a؅?_ý)§n?\îÎá™Gm?_ý)§n?ï³v/dÐ?"Ñ
×_Ÿ?ƒ"t5:V4?"Ñ
×_Ÿ?ïÉ©c*
¯?€rßiB?{+NQŒ~?€rßiB?îdêl^¼¾?"üOaáF?©±Y8\f(?"üOaáFAGN4FGL J1110.5-1836¿Òp B¯kØ@CÜ­¡À9ñb‹"À<0îP«?@ .l6˙?üo"èbT‰?À7¡?Æ!w±<y@ûB±Á¯@š#SAE›?êéTWp)^?äšs´,Â׿à´uBwHâ¿Ú{Ϥmˆ¿ÞìTQì¿çGpÂ_ágAGNbll3FGL J1110.4-1835CRATES J111027.78-183552.6?ïü…"
ì?9jak9r??ƒÒh¡§8?9jak9r?ïñÐå‹4§?[ÛÈùš?\^5Tʁt?[ÛÈùš?ïìÓëz?YúJÝÀÛ?c,¼íµ?YúJÝÀÛ?ïéÕK¡i?M &£v?f*´Iù<O?M &£v?ï÷ƒ+™?Gw"Š=½L?Pùªx©|î?Gw"Š=½L?ïª	(r»?'÷M9{Å?~ªûvÅb'?'÷M9{Å?勞¦ "?‰þÇEe?†Ôt	ý?‰þÇEe?ïŘÁ`¾?icTœ?}3Ÿc5ñ?icTœAGN4FGL J1111.0+3542¿êÌc#'z@PÁ)^ž	À;Qχ'0À<ݐ8ÇǪ@ BÞ£Žåá?õ?\l¡?Ý8LA÷ò?ïñð"<jê@ϵdÑ:ñ@Æ¡Íš¨?ï¦Vv.Z†¿í³Ç™kv¿Ê¨# 8Ü¿ÀœaJÙ«¿èÁUj• ¿ìcõrÞCîAGNbllFBQS J111056.8+353907?ïààµ.lò?tÑ./
(&?oJÕ²•¼?tÑ./
(&?ï²Þâ׃¾?ò
[Ú²™?ƒHG<` ­?ò
[Ú²™?ï{€—Ñ)?"›Ù_¹@?ŽOçÞpð?"›Ù_¹@?í—ÐGÅU?šÛî΋[?³GÁç–Ó?šÛî΋[?ïmâÉÊu?"åkº@?'_ƒ¡ŸGe?"åkº@?ï]ÑÙôJ?¢ùŒúHß?"EļOT'?¢ùŒúHß?î¯NŸþÁ?œªŽK?¥ü¤Rq?œªŽK?êôû‰<˜ü?´o'¤=ó'?Ä,Û
œ?´o'¤=ó'AGN4FGL J1111.4-4624¿íóÁ»;Ø@*œÜD9À: Ô`?ùÀ<-±2ã@gò'"ï@Zp?Ñ_H$†òù?ѵ"2E?ýü+_)[C?þû0ˆ!¸?ã¶i´Ï€¿çàæ_E	õ¿é–'q¬ë†¿â¡¬­O"¿îÁ
F9 5¿ï6¹ÐpÆ<AGNbcuWISE J111127.39-462504.0?ïªw†ZˆÉ?†/æc®W?…b[Ÿ]à?†/æc®W?îí«š€§ä?¢ƒÚ ºŽ?¡%F[e¿?¢ƒÚ ºŽ?ï2>Q?Œ‹»<4X?œÜ™´Ì™Ú?Œ‹»<4X?ïâ$'ž'?{cœ*?œ»ró—±?{cœ*?îW'´Öë?ª¬¤þÆ|Î?ª†ä¸¶FL?ª¬¤þÆ|Î?æ (e5-?ÍcȞ·2(?Ò¿¯5•Á¦?ÍcȞ·2(?ë?"W÷@q?±þZY)÷Q?Ãv "þ:?±þZY)÷Q?çœÙ Mp?°OõdBÙ?ÐÆL¿e?°OõdBÙAGN4FGL J1111.5+3455¿Î
J¶‡'@PÒ¼j~ùÛÀ;pZÇ̲ÌÀ<¡`†R"ø@"Ç~Õs•?ûr
—~?ÉüšoØ¿[÷7	B?{yïÃê@€(R¯zW?ÖIë;LÝ(¿ïþåþ÷í7?ïÿüÚ±'Þ¿Öøè^£¤_¿Ýî2BrkW¿å»l°Ú(AGNbllRX J1111.5+3452?ïþgåÚÝ?«_鮃d?)Ññ|`B?«_鮃d?ï÷8­_c?S[ ëè…ã?QŽ¥¿«Æ?S[ ëè…ã?ïõÁçÛ4Þ?Bâ5#TA@?T|0½	"Ð?Bâ5#TA@?ï묇±×?UVZM~?dSxü¬À"?UVZM~?ïþqR±0m?µé°ÒKW?(êл٠¹?µé°ÒKW?ïÛt¼¯7)?vDz¨o¤Ã?rE¡Âs?vDz¨o¤Ã?ïùŒ&½Y?]ÙJ?ˆA?IϞ±Ò/æ?]ÙJ?ˆA?ïÛlë–o?fº–n±r?rI°ì¨$™?fº–n±rAGN4FGL J1111.8+4858?ì`~h÷Ìf@Nu>ÄaÀ;׳¾
ëÀ=µš &@!Yy²s…3?ð4Âkñ?çÒÕZ::?ßê^bá̎?ôéËº~@ò00õ@^?ïø÷Bl64¿â~p·'©¿ïÃC·õf?îVų-¿Óm'©èò¿æjmAKúªAGNbcuSDSS J111158.89+485701.4?ïüëAƸ¥?@CæÓ«ë?8¥óº¯?@CæÓ«ë?ïø65NÉð?R7$€§("?O'*"ª°0?R7$€§("?ï£\ör"ú?ƒz–Î%ûÝ?‡(ÂfÎ]t?ƒz–Î%ûÝ?ïÿ¶'2S?~µx)Ô?	,Ð÷?~µx)Ô?ïüíú¢{ž?<B²Ù‡²?8,ϚÎ?<B²Ù‡²?ïÜøö:H??r
sx'
?qƒ"Ãïdš?r
sx'
?ïĤV$éˆ?ƒAgD¯÷È?}­ÔÖÝÐ?ƒAgD¯÷È?ïþŒ%Egq?)²j4E?'=§ú'j ?)²j4EAGN4FGL J1112.4+1751¿ë‡V¶}¼@PX£/D'*À;%ö4À< ÷ÞÉN"@››``"@ÄɅðoi?¼Áw녿´ÓœIÍ('?ûdÏÃ!R`?þS…~»÷¿¢-ï7Я¿æÉ	><Þ¿åü8§ç:¿Üg&Ɖ½¿í	}£~?çœÂñAGNbll3FGL J1112.6+17491RXS J111224.2+175131?ïôò´Ï?Q¢¡zKé?WúÐNü?Q¢¡zKé?ïÔ黽RS?xZ{®š…C?u‹"G˜?xZ{®š…C?ï´{ðfYü?šû÷Ž=¯?'áï†ì?šû÷Ž=¯?ïÌ­ÔÓÆ*?eCÐKÏ~?y©sÀÓ+?eCÐKÏ~?ï˟QR?u"šê»ú?z0=9©¿?u"šê»ú?î7Þ½~êÛ?±DJ&§¥?¬'$¡¶N?±DJ&§¥?ï­ZdjI?‡Yþ¸¨	?"©™&ýÒ?‡Yþ¸¨	?íKÃÜcC?¥ÎÖÉB,4?µ§Yáåê?¥ÎÖÉB,4AGN4FGL J1112.5+3448¿§Í*0NS@PâBؤUÀ9L p¸ÏÀÀ<!@ÏÓèJ@Œiƒý%/@ô¡ã6ï?ªÉSE¢Kš?›Wߺæ@$ñÃ&ZÞ@eMÌg¿Ó¼¦Ä¥`ø¿àÉqޔ a¿çˆ	¹½%¿éœ
V›¿éMnÂs-¿ïçâ!´†AGNfsrq3FGL J1112.4+3449TXS 1109+350?ïüî$"ç?3ñÖôÒP??èŽìød?3ñÖôÒP?ïöšIur?V—wúI?SÖËÂKj"?V—wúI?ïÏP¢QE?mîÑ"Vm?xW®»àX?mîÑ"Vm?ïû­€+^~?,è>±3 –?AJ/8®?,è>±3 –?ïõ²I=á?PYÁ3U?T›mïpµ{?PYÁ3U?ïÖÃìÜë?z7RµV#þ?týК\?z7RµV#þ?P¼—1?ŠlòÑ×F?‹TëÍj—Ô?ŠlòÑ×F?ïï`€HdÉ?Q΅÷ŠÂe?`Ÿò´?Q΅÷ŠÂeAGN4FGL J1113.6-1920¿ïû¶r'@Bë ¾Q	À;›r·®À<"‰†üÞã@|€3>q?ú''Y4?æõ2ôD
?ØbëóÁ{?õú%zãËí@VɩתK¿¯¯EAA'›¿ìä>ÙY£
¿»ÔyŒ]ò¿àMt'yè¿ïúïàM28¿ïÿÿ>¹úAGNbcuNVSS J111348-192252?ïõgbå¨f?uÿÿ¡Ú´ƒ?U1:2T\?uÿÿ¡Ú´ƒ?ïô¤4Û²v?Xéô ˆì?V·–*^ƒZ?Xéô ˆì?ï$ú$Á!ë?Œ³ÿð*?›`»kK^•?Œ³ÿð*?ïú•:—ß
?2!""à[9?E«ø`?2!""à[9?ïûRS+mŽ?NöšÍµxÈ?B¶³'2Ê?NöšÍµxÈ?ïÔ^ۜb;?|E½V?uВB>Ø?|E½V?ï2uÍÙß|?"éå|ëâ?™±F<-
ƒ?"éå|ëâ?ï÷J³=À¼?B}€¨-2è?Qj™¢»Ï?B}€¨-2èAGN4FGL J1113.8+1528¿ìS+ºÝ¦@P!¼ÓZ…ˆÀ:õ'R}À<˜s%³@k֒ÉEÚ@Ì_¿ƒ8.?ÀÞº z^k¿¦âSÁÊ?眐úŽ¦÷?ùræ‰âA~?ï›îs¿ìCÑ¡ð§¿ßJ¨/^']¿ßæèArf$¿äw4cn¿ß-¿ÖÅAGNbll2MASS J11135586+1528058?ïû9NÖ&é?8'{?CÅ<`9v?8'{?ï×ûF)Q?zZéé'Ì?t\ÓIüi?zZéé'Ì?ïÚ}Cä?xŒBœq`!?rÁp~¿aù?xŒBœq`!?ï³àvðÏ?g
üÕFY?ƒâDQÂV?g
üÕFY?ïñžÿ¶ü?RJa2¬óç?\ÃS¦ó?RJa2¬óç?ïH¸¾Örœ?™fŽíR°$?–èè 
B–?™fŽíR°$?ïÞi|gÑî?x˜h'ðË?pËAڅe?x˜h'ðË?í´éVE\?œñoÜkW?²XµOúá€?œñoÜkWAGN4FGL J1113.9+5523¿ë.=øU‰@LX[žŒG¡À:Ÿð+oðÀ<ÎeÅV¶Æ@ïÑÃ=­@]'Z
7'?À)§Ù£Iò?¸HÈEÔv?ù@ùª{i-@¨âºtÛt¿çuB!b¦?°'×5[†¿æeçñr¿Ô:Ð`€r¿ãž"Ք¿ï÷އŠMAGNbllSDSS J111356.29+552255.6?ïýðyáS©?-µˆ¦—ÚÙ?0|0À›íþ?-µˆ¦—ÚÙ?ïöE°c`?OÁĤ¹]?St Ç¡n?OÁĤ¹]?ïô÷Pa ?b	¶~Ðá?WÎÝ®_?b	¶~Ðá?ïëºcÇ-Y?EÊÀD¬º!?dEœ<ò.È?EÊÀD¬º!?ïý1ïfTÉ?0e;ØÓ?6p†•¥Ø
?0e;ØÓ?ïÚðHšg?s<ûä(:?r‡òÛ²ÌN?s<ûä(:?ïïÞÖÿDˆ?lñ*-ß¹õ?`!(¼HV?lñ*-ß¹õ?ï¯ÐÆ!–?p*Áo*–?"ø
X¥?p*Áo*–AGN4FGL J1114.5-0819¿àÍAý®õ@G¾Cªy»®À9ԙœØXÀ<+£<±@<Áz^?ü@CßâSG?ºÖ<!ÄJó?ÂL;ÂÎÇ#@­·®W–À@@à$ÃXÛ?拝'uß¿çƧÿ¸ÝW¿ê)!¯íï¿ìäÐ.Ë¿ï¢£Y6¿ë¾hêAGNfsrqPKS B1112-080?ïûËùW?A®¹ý¸r?A¿µ'·¶?A®¹ý¸r?ïîVœ¸ª?]þM·'¦Ú?a©ôz¤­'?]þM·'¦Ú?ïÕ¨Šð€Ó?q_KßM8?u+º—Ê1?q_KßM8?ïÑVÛI?aêå´ø·6?wvTœÄ¯8?aêå´ø·6?ï෎)×r?mpÆy:]?oHqÞg?mpÆy:]?ﴟsŖð?'î—W‰ü†?'Ø#«H?'î—W‰ü†?ïq»n«"S?Ž¶K̟9ó?'È'/¶ß¢?Ž¶K̟9ó?î´(á)	?'A©a?¤½qñýn?'A©aAGN4FGL J1114.7-0248¿ìG'#©Rt@J¨~8ëÀ:EÏÞ²À<)œ1úN@&¹¶ðl@òÊ!÷¡?ÃúûHáb?¶y"˜€•?ð™šäó?ÿàTyá?ÖBˆCa¿êÉԕ*™¿è±5Ý\'ü¿çӄ¼¿ïý¸'gù¹?ÊöÖ-ɒAGNfsrqPMN J1114-0248?ï퇏ÖÍ,?c›¥rø¾k?bxp´´U?c›¥rø¾k?ﺁ޼äL?†¿(	äyJ?_ˆ`=*Î?†¿(	äyJ?ï¤OæT?€''f½R?†ìnœ$j?€''f½R?Ï(ê?t<`6?‰=»¹™?t<`6?ïæ*,ŠˆÁ?n*o2"	?iÕӒS÷?n*o2"	?í"âÁ3o!?¹€æ(P'?³`é÷@mø?¹€æ(P'?ïY¿Ámëb?=$§ù¹?"ÈЊŷ?=$§ù¹?ë<÷\ëù?°Ì•@)Ìé?Ã"ÄP?°Ì•@)ÌéAGN4FGL J1115.2-0703?ÑÚ'ä@HQ^	À:XaÀå8À<Lk"ÌÐÿ@ò;"™¦@@"Eð?ºÒ6™A?¥&¨$:¶¤?çވì£+ê@ÆâCV–æ¿æƽêî¿Þ.dß¾—¿åÎÆ×ÀEÖ¿à-î$nt¿çéŸ"w¿ÙÀq_=ÓAGNbcu3FGL J1115.0-0701NVSS J111511-070238?ïþ0Ê£&á?%œR¡ðj?,óVšG(?%œR¡ðj?ïô
büÆÝ?Y%'ÜÃÚ?Wë9ðtÆH?Y%'ÜÃÚ?ïöür?`l"ò£•?Sî)Fú«?`l"ò£•?ïø=ÈÒ0?8wûa¨À?O§ÌÅÜD?8wûa¨À?ïûkÔuŸ?:pƒß"ÃÑ?AÂQfáP'?:pƒß"ÃÑ?ïÌ×aêð?€xÌþt‡`?yö"G{cÖ?€xÌþt‡`?ïðē˜M¿?g~wZ!°?^vÙ:˜Q ?g~wZ!°?ïÜo×m)?aLÔõZz?qóGø̋Þ?aLÔõZzAGN4FGL J1116.6+2915?ì'<Ë.ß^@QB­­ê‰À<Kl»êý9À= ¤&ó@#¨©Úî¤?鐗ÈAî?ép›Þî7?ê~e`¬é@"ÄæN~@üiÙ¿ïÿùSt?ê‹ùæ/t¿ØÞ|øy#?ï¡æڕl?Ì«IYæ%c¿Ð2":¯ÔDAGNrdgB2 1113+29?ïá3³O'ý?š
£_$°?nÌL—°ÒÆ?š
£_$°?ïó"ÛW»9?b¯f·#€(?XöI¸ý­U?b¯f·#€(?îÖ8o*õ?™IóÜ4?¢œv'U'´?™IóÜ4?ïúАўï?A†J—½¦?D½»¨ÖzM?A†J—½¦?ïÒ4Þ. ?'—‹Èƒ»"?våÛâkÔ?'—‹Èƒ»"?ïÔ@+"-t?}AR*™H?ußêHw)å?}AR*™H?ï0>¿¶íE?"m!÷"Î?™ø('óX?"m!÷"Î?ïñ5·>g'?a‰ÿ¢~ñÖ?]"'Å)]N?a‰ÿ¢~ñÖAGN4FGL J1117.0+2013?êk€«zÜY@P×j~ùÛ#À8úùåܞÀ;ï*¯ÖòÀ@9 Va¶~?ÿH"¹7Ē?¤œ|^0ž?Q~'œRç?±"÷¦À½@±pÿÇuö?ϗ#k"ù¿ããpè gê¿áE†òÍè¿Õ掿ËÝd¿äο€³ï†¿Ð.feÍxAGNbll3FGL J1117.0+2014RBS 0958?ïþéÿQs)?›_Å'M?!`
"YyQ?›_Å'M?ïø2ïÊ{?Sc÷íÖ|?O4@øY—ë?Sc÷íÖ|?ïøÕ Ÿ·?=˜î l?L©}´D†Ù?=˜î l?ïÿŽV«™ˆ?#¤D¨U?jRÖÏ2?#¤D¨U?ïÿ1PÙ·?™\«ØX?ÜûÓnTÄ?™\«ØX?ïÚöQ8ç?uIBæBãT?r"×^Vè'?uIBæBãT?ïú<ng´?MÿG¨ÏÖ?GG$YŒ?MÿG¨ÏÖ?ïÿ¬d͐?AüÉ3Çý?æÿ[½"?AüÉ3ÇýAGN4FGL J1117.2+0008?¾ÊÌƱn'@Kcí¿‹›ªÀ:÷k:
½ÉÀ<Š|@Ã?@ ¤É'PÑÕ?üº¡6F
+?Ë­=¾§p?®|>>ÿð?â®q,"@µ+‹¿îÏõ@‰]?ïév†oj¿Í$¨ҿDžþ²"&›¿éÃl2š‡?֖K›ßÄ÷AGNbllRX J1117.2+0006?ïþ`
VÆ
?"'ÁŽJóÿ?)ÿYaõN~?"'ÁŽJóÿ?ïóâD(n?ZD	ð¯?X;wÂ/Ã?ZD	ð¯?ïâ Â2À?c'a°¡?m_âk(Ð?c'a°¡?ïõþúœh×?@¹üsU"¡?T
Ç.RN?@¹üsU"¡?ïý\ÊäÈË?0Ü]´5Ÿ‹?5ª?	~?0Ü]´5Ÿ‹?ïÒ׉zy?yÜï(?vö(´ß°?yÜï(?ïÁ|.¤® ?'ptÕÏ´?Aèœzä<?'ptÕÏ´?ïã¦}F—?_­ÙĎY.?làYr;I–?_­ÙĎY.AGN4FGL J1117.2-5337?ïÐãò+t@ÐO±;`À9ÜRX'hMÀ<HjÒܱ@¤ëg†ù?û1GÏ¢j?¼+‹tõ¡?Ì´ªV«2s@…Ìe÷@ºe+'÷?î©¡ÙY"¿ä
~q ¿ÓØe1]¿Óޖ"ì"¿á̈¿V"¿ïÿ'âH	.AGNbcu3FGL J1117.2-5338MGPS J111715-533816?íî¾7k?©:Áº"È?°ŠHƂ?©:Áº"È?퇒Ù6µ?µ¥€ôU˜?³Ãi5—Û?µ¥€ôU˜?îv.Æ^k?™±Ä4'%¥?¨ŸýdR?™±Ä4'%¥?î¬@=û8?™=gåN?¥;÷kÏv?™=gåN?豺+yDS?¾¦ì_?o?Í9Rî³?¾¦ì_?o?áM?ê«?ÑìØÎQ¡?Ýeè*©Õ?ÑìØÎQ¡?éù‹x)îw?¯Rš—ŽL?ÈÒXF#?¯Rš—ŽL?éƒÜóã?§¦Ç'kÌ?Éð¨1Àu?§¦Ç'kÌAGN4FGL J1117.6+2550¿êa·šÇ¨@Q@9Õä¤À:tu;ÄÀ<šk‹iU.@úGtª@Í]…U?º]âžÆ)E?Žê¾¶oÏW?Ôf˜:@YYBfê?î†òBR5¿âÂÖ>e–]¿ãæÅÒÈq¿ãµDD¿æہÁ
̸¿Ù¥W½×žAGNbll3FGL J1117.3+2546RX J1117.6+2548?ïö O8ä?n©K«^™è?R¿bLĈi?n©K«^™è?ïöH՘±?Q}¿º'Òô?SnTöj=«?Q}¿º'Òô?ïå5¼ò?wtGm,tA?jûÊëŽk?wtGm,tA?ïàÅ_›$?U9áï¼ðp?o: W&l ?U9áï¼ðp?ïç
•X±?cí|vôU?hüò'¦Õ?cí|vôU?ïØ¡[?tpXèWwu?sð/qjx?tpXèWwu?ïéÜjع?saÒە®?f#•¨7$?saÒە®?{¬@2?uŒ©¤V?‹^!€W•?uŒ©¤VAGN4FGL J1117.6+0217?æ8ôxë׳@LBŒi/nƒÀ:Èût€À<])4¬¯÷@S¹¿~Û}@ ¶fXúm?Ä\HUYMÏ?B»ÆÇúl?¡Þ.ÁUí•@gÕR­Kþ?ïtŠˆ×¿â'~e'¿é´*¿qD'¿ÕØO¢T©%¿ë8ë¹4¿ïñÂàÍ=AGNbcu3FGL J1117.7+0217PMN J1117+0216?ïûúٔJ>?;Fa3Oõ?@˜Ê$;Ã?;Fa3Oõ?ïó—âèˏ?Y7ýèæ˜W?XÐ9Þ±óK?Y7ýèæ˜W?ïæ")(K?j¼­l®?iÝÖÙל?j¼­l®?ïõÙ¹¢×?<Hvû'Â?TLŒ–•ôð?<Hvû'Â?ïð&¬ù.?]¸ÅÐÏ{×?_²¦R\Ã?]¸ÅÐÏ{×?ïÍÉ-tÇ?†o,€?yi#ðI#?†o,€?ïéË.MV†?pø å@Ì?f4ћL!ñ?pø å@Ì?ïÖ'œ|"?bjזÔì?tì1«ñxd?bjזÔìAGN4FGL J1117.7-3650?ïì'n…wV@6Y~™cõÀ;òø°€fÀ<"ö(æ©@Ҏqó7p?üãx«ˆ¤?Ôo›-îOÔ?Ó.¹PïÝ?ûUȤI @}´üvˆ?ïÌʳíض¿é0ç"øoé¿¢è&šs‰:¿Ý[5ZÕ¹…¿î¹Þ]˜âe?ÕX@2õö'AGNbcuNVSS J111758-364918?ïä|7DK?a(ܦ2Q?kƒÈõnUð?a(ܦ2Q?ïޗIªY?p}Ñ8?p´[zu?p}Ñ8?Œ!?ÑfÃ5œ?ž
ìŒ6­Ý?ÑfÃ5œ?ï¬ù^apo?k%êê¶?"Á¨k€X?k%êê¶?ïÚ£­Ò_?p€–ii 5?r®){Õà†?p€–ii 5?ï–]œé/Y?Œ0ì€&?Šh˜Å´)¾?Œ0ì€&?7®\?šm"1Ÿt?§ï–ô¶=?šm"1Ÿt?î»u)ye?ÿU߉F?¤H¯­hi²?ÿU߉FAGN4FGL J1118.0+5356¿¢ºýÈfbj@M¬ÿ§ëlÀ9†S³Ü;À<"û¥'l@"J"ú?ü‰ÔÊÈÏ?­Ÿ¶¿Zð?²?Mȵ»ä@_íQx™@‡k'–Fÿ?ïÐnýäœÍ¿"
ñ)¥…¿àWŠáÅ¿×h^ùŠšù¿â.î%)¿Ú½_œr¼áAGNbll3FGL J1117.9+5355NVSS J111757+535553?ïú¶SûD?Aä›8E—?E'ÝùŽò?Aä›8E—?ïتؗ?tõÕB[×?sªõÜ@€I?tõÕB[×?ïêå0hJ?c˜É©n†@?eÏv¹²v?c˜É©n†@?ïUÞ×r"?tb³?'~?•D%&ˆ³v?tb³?'~?ïöL›l¶?P*´X+?SfɌHFÄ?P*´X+?ïo—½?–d9+?'­pçu?–d9+?ï½Îî¡D?…Þãi‹"Í?€ŒDQ×£Á?…Þãi‹"Í?íxÉÞc€¶?šÔ‹,ûRö?´9±
¾8Ï?šÔ‹,ûRöAGN4FGL J1118.2-4634¿åÏOë>–­@*«nø_»À:ZëÞàÌÀ<3ˆ˜`´@¬Q'M›@TªFJ?Ñ4òÛª5H?Ú$&»U¬@1[µˆ@(t,vÖ?ïövêB(™¿k»Ý2Âí¿çòCŸ'Æ¿æcçeÕFï¿ç]13~²Ž¿Æg³'ùÄýAGNfsrq3FGL J1117.7-4632PKS 1116-46?ïówz¤¥«?W?ÁEÆ?Y
yZ?W?ÁEÆ?ïÑЅq¢?|–!­¸T,?w½Vý-¹?|–!­¸T,?ï:A·QÝ»?Œ³ë¹ÓÊ
?˜·É3ä¦?Œ³ë¹ÓÊ
?ïØ·'*?YÚÔLì—?sõ$E3Ú±?YÚÔLì—?ïò¾bô
{?]Ä£[*óE?Zƒ:oÛ	Ç?]Ä£[*óE?î¾\"÷¹?ª…P¦ã?¤6Ãþ n?ª…P¦ã?íûègœ$? 'Þ‰…?° ¿ãyDa? 'Þ‰…?î0HÌïÔ±?™î;œ?Ý?¬ûs-"ô?™î;œ?ÝAGN4FGL J1118.2-0415?ﮃ¼ô£½@I²@(äüÀ9¶<ËbjÀ<z¹ÚÁ@ †ôü@Ù@ÍG¤ç?·ë'ˆþì°?¶¤?	ˆ?ù+õQP@|@BeU¿Ú rÑ®³Ý¿ãá01 3¿è—è¿qšw¿çœ'aï‰:¿ìÓfQÒ[¿ï"Í®oêAGNagn3FGL J1118.2-0411PMN J1118-0413?ïüï:¶h?HÇÐIr?8‡éÍ¥?HÇÐIr?ïóý•4I?\À¬G?Xóí·?\À¬G?ïèºàã?eƦ!Xê?géE¨
‰?eƦ!Xê?ïÿyœD¼?n"ú"°þ?Ü4Š}rI?n"ú"°þ?ïþ&dKb?#Á7äZA¿?.É:E¸?#Á7äZA¿?ïÐ7bÂÂÞ?wìW¾A‹?wäNî¥&?wìW¾A‹?ïᷖ•êI?r·nÀùÂ?nHiCšq?r·nÀùÂ?ïþ¨.)U†?.(ò\µx?%} e·>‡?.(ò\µxAGN4FGL J1118.6-1235?ï%7‹BÏï@F*䎊qÞÀ9öñûÀ<;Æ*\}@ÛÓöeM@Hæùž¼ï?¼±;aU"?Âj‡ÃŸÒ@	Ĩa³@8÷¯#™?ïÿÿÊPË¿çîG;'ô;¿ê|Vþ–¶¿èӃÕâö¿ãÏò@Ϩõ¿ïþ,UÉ`1AGNfsrqPKS 1115-12?ïüÔ_":?8ÕKxÌ l?9_Œîz(?8ÕKxÌ l?ïê#èÆ;?d}Úbo?eÜku$µ?d}Úbo?ïƁ4|?}O¨ð0Í{?|¿uŸâ–?}O¨ð0Í{?ïÔ¨3˜çK?_@`Ð÷À?u«æSØ®{?_@`Ð÷À?ïïpg_úU?k[ÊX䪲?`˜ÖÿjT?k[ÊX䪲?ï™àº¦•½?‰º´í0?‰‡Ñ`©dÈ?‰º´í0?ï)"˜Ü/k?"Nb
?šÛ¬æ1à"?"Nb
?î¥má–Â?" SÅj{ö?¥©!æžsã?" SÅj{öAGN4FGL J1119.0+1235¿í'Ùž8Ý@Oø·`,'À9íÝ{p¹¦À<Þzt:@%ÿµØ>›@=ðüVþ?½M6êwØ?Í^#vҚA@3xî(g'@
~w)W<¿ÂäÏw÷ÞH¿Ý8e˜º¿çÊ3ß3W¿ê¿cW¾-¿ïþÖj€˜?î§<_VÒ AGNfsrqOM 127?ïíxÿεc?^îŒ	Ã7?b‡ÍD?^îŒ	Ã7?ïó'"Ô:ª?[R{•ÕV?Y°öºjá?[R{•ÕV?ïfÎk»îa?‰Mcx?"&2Š:ä?‰Mcx?ïóÔ
2îj?G>¡á<ï¸?XWæVûÀ?G>¡á<ï¸?ïäBi?k²Ç~¶i¶?kóoŒˆî?k²Ç~¶i¶?ïÂ&É ûì?@è"l?~ì›'òå÷?@è"l?ítҒ‰"ù?¤Ú'©ÿG'?´Ykiü
7?¤Ú'©ÿG'?ïX†åóö?|˜Idn±?ˆ©ÞCfi?|˜Idn±AGN4FGL J1119.6-3047¿àT‹ÃÔ<@<ÈæŽ>óÀ;c…LXžÀ<´)3Õðb@"/sš×\?ü8ÇÃ?ǂ´eLàÙ¿˜Du?Ò¼Ú;uL@'®¨—›¿ÕÀæå|Æû?ïÜE É
пë{;	ÁJ¿µ59È£T¿×ö‰Ÿ%Ÿ¢?țt$¿ýÜAGNbll3FGL J1119.7-30461RXS J111941.0-304652?ïþ'ÕTR?&AºÿÔ?.gÒîæO'?&AºÿÔ?ïôÃÆ=ç?[:šð1Ý?WÎx²½Ð?[:šð1Ý?ïâ|r¨zC?s.wáßÀ²?mƒœ=ìR?s.wáßÀ²?ïüùÜ'€?&µÃLç΢?81á2ô»?&µÃLç΢?ïù.}ýíè?I/·QÛ?KF´+‰4?I/·QÛ?ïÒn|4"?wµýJ"‰?võH½Æ6?wµýJ"‰?ïÛuòþî;?x½»½Pòþ?rE}É2§?x½»½Pòþ?ïñý~£ý~?S½‹%_xr?\Oãõ?S½‹%_xrAGN4FGL J1120.6+0713?ï€/úˆ`¦@NV0U2a|À9ä(rÀ<P)Ôà@˜à¯à«?üÉçÅv—6?¾Fa8T/W?ٟúdŠn@XÿI Û@ˆj$aY¿éŠÐ=š•B?Ð6¢~oœ›¿×>adžæ
¿â¸J"xÈi¿ïÅ<¡?ßjÊÄ^êAGNbcu3FGL J1120.6+07131RXS J112041.6+071335?¨s-vÀ,ª?³«:V«?îxÍ(½8…?³«:V«?Ö7q'×׺?ÆŐ*ãŒ
?ääGl#?ÆŐ*ãŒ
?Ê÷8«Ã?±ÿØ-w3?éB:1Õ<?±ÿØ-w3?äE0·¿É?ºSxß ?×užöm?ºSxß ?‡ä×å'•?œ¸ÜV·Ú"?ï l My?œ¸ÜV·Ú"?°ç²·*'?®¹²^y—?íãÉ©°?®¹²^y—?£G™l"*?–eø''ƒ?î΋†[yM?–eø''ƒ?¶‰½µïµ?©rá¼ —?í.È\ûƒ™?©rá¼ —MIXED4FGL J1120.8+4212¿ÌF ;ÁU@PŠk΅3±À8ÁA÷TðÀ;¦. |w@ ¾ØÈ.?ùÀ¿xPt?¤wÉ¡Zii?§`®>@eŽšbv@tmoïüþ¿ç'E'ƒ¿Ï²¼•ÇýۿՄ½A¿h¿ÕKí^'²u¿ÉHY`™¿Ñ+¼üKAGNbll3FGL J1120.8+4212RBS 0970?ïû6ÈûI?9|ϲ·‰Á?C$܅üA?9|ϲ·‰Á?ïãÑ©*†;?léÁó}'6?l.Wòä>?léÁó}'6?ïûáž|>?˜f72I¾? ƒÇ	S?˜f72I¾?ïs—"­?yÁ«b2:?'í$Ad
?yÁ«b2:?ïäòåUI?dÞïbƘ.?k
ô
,—v?dÞïbƘ.?ƒüí?''8Æ'é"?ˆPßBO˜µ?''8Æ'é"?îø\'ü¦ã?˜ô'RlMJ? z=~}Ã×?˜ô'RlMJ?í¯Ú/®:Þ? ÕU/Òî‰?².²B? ÕU/Òî‰AGN4FGL J1121.3-0011¿ïÑÀeúõn@K"Q´þÀ;ËñºzÀ<œdÐd1@ Hƒ}Îaø?ÿ"à°«.?Êϝ÷øµ?ŽÚÜs͛î?Å£øSY@ҍٜéÛ¿ïÛO¡ÓÏË?ïý…Ò<xV¿ÛeD¨P—¿ä6"Ü¢¿ÃÛ-¸Ÿï¿è;¿(Ÿ[zAGNbcuMGC 0019706?ïþf+œÕ¨?½xU<´)?)G¡â$Q?½xU<´)?ïôxï™Å'?XÞä¹<öû?W!n0ù?XÞä¹<öû?ïëCÒµ?[»i®ø*?d¼-B°`$?[»i®ø*?ïú.Òå5?3sQ±·#?GD·y-ZX?3sQ±·#?ïý9.IêZ?1ÖdGY?Ò?66Ž€{öÂ?1ÖdGY?Ò?ïÈÃN…r?}äގ_?{žXʌJ»?}äގ_?ïä7Ïï?sʔÿ¥ÿ?kÈ0üX?sʔÿ¥ÿ?ïçBô"²œ?_£ª‡…m?h½Y"Ù?_£ª‡…mAGN4FGL J1121.4-0553¿æ%ÖқT@I9PüqÖÀ8¥Q­DqÀ;Ï×ð}ñ@¡sÕB<@x"¡¸?£À–2±Ù?Á£~õ©dé@Sžã…v@ƒaòåæ¿ÍýV
㘿â°]ˍ1¬¿å*Ú~çÆ¿æÀ–]¤öÅ¿íƒ|V'³Ì¿ã$A"àAGNfsrq3FGL J1121.4-0554PKS 1118-05?ïõ"jÍ9?P²áK¯_å?T÷*?P²áK¯_å?ïê%3|jp?l1ë=…Üu?eÚÌjØ`1?l1ë=…Üu?ïmB*C?ÖZåà·>?'^÷²(±¥?ÖZåà·>?ïõ¾8	†¼?@iMSbɁ?TƒÔ5W>?@iMSbɁ?ïå…}$e\?d­ÃÍÈ?jz'ÞZSŠ?d­ÃÍÈ?ïŒü°Y?ª!,3Zb‡?Œú€Ðzd?ª!,3Zb‡?ï†V¶1?¯xlçù"?Žzꊀ ?¯xlçù"?ï¿Ù.+ü?m9i»h9?€	¾¿sÀè?m9i»h9AGN4FGL J1123.1-3233?êóÆ,¹`M@:¹Ñ¢£YÀ;–m•/À<žÉ¬†Ü(@Rž˜†ôü@óý]ŽP?ÅÁ¼"…ù?‹†ù?Èòüvރ®@‡A 3fµ?î=ï^òÿ'?ï§$f畦¿ì)õœÏ®ÿ?"×Bz+Æ¿ÜKóÞßsî¿ïÿõž}.)AGNbll1RXS J112318.0-323219?ïü×ÜA×2?.d‡»F?9A1õÈ5?.d‡»F?ïó#«"Oƒ?Y帛…^§?Y¸©kªA?Y帛…^§?ïã
qÖB?pݤü-ø?lõþ©¦‡?pݤü-ø?ïú¤°Îê?10‡•^Ä*?G…m¡ì	-?10‡•^Ä*?ïõFŸæS ?S©«Ÿ~Î?UrÀ¤îº?S©«Ÿ~Î?ïÎq1£?{Ý»ò[ë?xÇwiî,*?{Ý»ò[ë?ïÔ-T}?yd(à%DŠ?uÀi;Ö¹k?yd(à%DŠ?ïëׂÄ|-?ZŽXxêÙ?d(}è«´?ZŽXxêÙAGN4FGL J1123.4-2529¿ëÌ$á
ò@@£Þzt:À:´É.4À<Q¤Æô@?ÿòˆJ¼½?Ë,Xãñ×s?Ó¢šÛ¸ù@j[¾l·¹@«_ð«y¿î´@ÿ¤n?ïý_;Ϲç¿âFr«G¿ã¢$'–H¿çêèÁŸòú¿ïÿß~€8 AGNfsrq3FGL J1123.3-2529NVSS J112325-252858?ïúҗù¾?A"gužé?DµŸ]#W?A"gužé?ïò
F˜v?[¶hM™€b?[ås'»?[¶hM™€b?ï­èON
¿?|Ütóº|ß?"…ì/ììM?|Ütóº|ß?ïî 8?FŒI–S>?aøàugç?FŒI–S>?ïû=#³·?BôܵÂ:?CpÇė›?BôܵÂ:?ïÊÄgŽ–?yò[sƒ?zü6;5>?yò[sƒ?ïl¡^½ƒ6?ŽS8Zf2L?'kÔ#(/;?ŽS8Zf2L?ï¸Õ4¢ì?q_ë2ø ?Ê»õ–ôé?q_ë2ø AGN4FGL J1123.5-6418¿Ã™E˜:ŸÀ] Å®À9ªkµZÀ@À;)Ì¢Ûb@¥'—H±@EKc¬?Èaq	,¤y?¼ðò›éU?øyìU(Q@¡¨ä»+?ïÿP3:¿â¶CÞÒõ¿æä%®æ2¿ì	tÞNTw¿è(úà†h¿î–JŸ‹vAGNbcu3FGL J1123.2-6415AT20G J112319-641735?ïþ¿j'æ? ´´¸Ó×?$	[ìÊ°? ´´¸Ó×?ïêã´M'?q¬
ÌÛ?eK¦ʵ?q¬
ÌÛ?ï°î˜W,ë?ƒèƍD?ƒÄY딝5?ƒèƍD?ï÷½AG%·?5J.Ÿ+–ƒ?P…}Mø¢9?5J.Ÿ+–ƒ?ïþvc8?,їë]Þø?.ȕxJ~G?,їë]Þø?ïbÆ>›Ï²?©~
õ`ñ†?"§8%¦Ñ½?©~
õ`ñ†?ïÃØKIï?–µU
>4~?'"ñoX"?–µU
>4~?ïÈSÇ@5?kÓö?j²?{Ös>s?kÓö?j²AGN4FGL J1123.6+8028¿´~F
ø³}@AótÝÛÀ:Øý›²yÀ<ÍK
P¼@o*|«L?ÿ³vŸ™Û?ËO äüïT?Õê{´V^@>À·pD@ÖèÚt€¿î''¼¨'?ïùx&'JÈ¿å‹ZÜÅhT¿Ù'D:Ât¿î­¿jäz¿ïóHa˜¡LAGNbcuWN B1120.0+8046?ïÔºVþi}?s…ç­È(?u¢Ô‹Êx?s…ç­È(?ï¢8Š=¹¨?ŒHñ{üÒX?‡qÝ~P?ŒHñ{üÒX?ï	ð'šµµ?ž%£[½?žÁï¥Êw?ž%£[½?î¯T§¾Û?"j\O?¥
µ""vZ?"j\O?ï´A¾;d…?'&AÈÎ@º?'ïlWjÃ?'&AÈÎ@º?î~û@¢?±éß}…^?¨Î!¸@â?±éß}…^?ììNXŽÈ–?ªŠ{+ŠìY?¸<e¢K?ªŠ{+ŠìY?é²ð4?µ
Û05ÿv?É4?é‹/°?µ
Û05ÿvAGN4FGL J1123.8+7230?ïoچ§W%@EŠn~bÜnÀ;œ®¶aP}À=¡'Œ_@!¹üøä'Ì?øÃæÄŗN?Ê-˜),A?ɀ1©k@óH+è¼?õöA»6L¿ïÓèë"³¿ï¶R¢dCv?ïÿÂWþÅ¿×î]@L÷¿ßx`cíæ"¿È*ýD8êAGNbll3FGL J1123.6+7231RX J1123.8+7230?ïøùæWÚª?IÔ8ùe'?Lež¿vì?IÔ8ùe'?ïºÍø,2I?Œ7íy'?Lôóm²?Œ7íy'?ï´Õ;Ӎ(?ƒ…Â×ÈU?'ʱ
Ô?ƒ…Â×ÈU?ï6´÷á	?ƒ>¬sõö?™)n;Ütí?ƒ>¬sõö?ïùÛæ<¬Ñ?Cv;Ž¡93?HfvÚE?Cv;Ž¡93?î±o~»Œ?³¦Ú¬«¼~?¤éˆð.E?³¦Ú¬«¼~?ï¯	Ûv?†í5‡}6?"8=ññþ?†í5‡}6?ìîÞ/´¬?ª9G¹û?¸‰,\™"?ª9G¹ûAGN4FGL J1124.0+2336¿Æp×tÃJ@Q~Æ"§À9ìú'è},À<-:ƒ‰ŒÜ@¹ö¾ëv@Bá¹Ãۍ?³ÌÕ±!öu?"Tµ ¥?Ô4ªžP8@ž{Fó.‹¿í'ó*ö?ÌÒE݄Õè¿ç$ŽŠqÞj¿ãi!Œ—¨¿ä
':ƒŽ¿çø— B•§AGNfsrq3FGL J1124.1+2337OM 235?ïýòÇ漖?$"ÓÛk©?0i¾Öí¯!?$"ÓÛk©?ïõݪô•?X';…øŠ
?TDª?X';…øŠ
?ïé*$…Š2?js/á
ÞO?fÕÛ©0}Þ?js/á
ÞO?ïïÓݍ9d?Ih£¢¶W?`,"¤@ûÂ?Ih£¢¶W?ïø1ˆì.?H`ñ×öP<?O9ޟàŒ<?H`ñ×öP<?ïÚ@¾È8?uoò4?rñ_¨Úó¸?uoò4?ïÄz—1»?'š#MQ2?}´hÒzT?'š#MQ2?ïµe>£1?rñãH‰?'¦¹aè×µ?rñãH‰AGN4FGL J1124.0+2045?ï
Óyus@QEy¿ß~€À;Ù¦ÏãÀ<¢­\Äüõ@ iZA"ö?þ*ål[?ÍÆ^ˆ¦?´¦ùS"{?ìzšï°@œ¶ü%?ïã_0пÔ3Éü7ôc¿ßƒ~O;R¿Ù*ü˜lrð¿Ý|¢gô[¿ç\ß¶´]AGNbllSDSS J112405.35+204553.7?ïþ"­éª?4 ƒ¹Ìn?&öÂÆÝ~?4 ƒ¹Ìn?ïôPÐ/¶Z?XÝ}+ŸJ?W^_Ym ?XÝ}+ŸJ?ï÷O€¬ôÑ?;Z®95c?Q`þŠ™}h?;Z®95c?ïê½I¾:?F?Zµ#ðZ?eBêȽÚ?F?Zµ#ðZ?ïÿèm"?÷ƒÀóªœ?>ރ©ƒ'?÷ƒÀóªœ?ïÓëÜK^½?|øɘKy?v
À3™°?|øɘKy?ïùá8н.?U#½¸?H{ø÷¬Ñ?U#½¸?ï´:2™_?où붖X]?'ñstê¬<?où붖X]AGN4FGL J1124.4+2308?îC»#,*@Q{€Ü3rÀ:ã¿Í
	nÀ<]RÁmóù@T1I#4@bÁ–8?ÆM8`C¸?A±=é/Z@È1ÉPÁd?æcq>†£s¿ì>!£¿¿çà¾áý‹‡¿Øˆ¯üÝ`Ä¿ÞyÌÑý8¿ðAGNbcuCRATES J112431+230745?ïýòeHë?(9ÿxߓÖ?7kqzÁ¤?(9ÿxߓÖ?ïõ"+ü»°?Y 	Ónùœ?T÷§ž ?Y 	Ónùœ?ïñý¿š"?i&M­Ä?\€fˆK?i&M­Ä?ïö¶t_'&?8ÀQ†½¡?R"5ÜôÎ?8ÀQ†½¡?ïý7°_H?1&Õõ'%?7¦A7'*ê?1&Õõ'%?ïÚkJÉd?rsÓ햆–?rÊZD4?rsÓ햆–?ïìԜ¤æÕ?v£×Kô'?c+cNº"[?v£×Kô'?ïÑQv•2­?fyÃæâ1?wWD¢(ÙÈ?fyÃæâ1AGN4FGL J1124.6-0809?ÝkL }ʗ@Hv <K	êÀ;MFÚ°À<tò ›ìZ@ AêÜs@…Ù ð¥ð?Ï?8ÇǪ?£&Î 		ê?Ք˜B±@‰;¿HÕ²¿âBRÑ^,¿æbP1ò¿èð›.£¿¿cŸŒ¢»+¿è=…Ò<xV¿ïîåüH»[AGNbcuAT20G J112437-080643?ïýÄåø˜?0՗ÿX†1?7ÑØk;ô?0՗ÿX†1?ïñœuŸœñ?]¯z´U¢i?\Ç`'
¥?]¯z´U¢i?ïæà>(d?q§{L"í?iÂ$¬?q§{L"í?ïóÒ#¢ƒ?<Î9Kô,l?X[ÿªÔ?<Î9Kô,l?ïü—9åKk?8à|3Á+?;F.·•|¥?8à|3Á+?ᄂÄ"·Ä?"ޗa?€VϨÅ?"ޗa?ïÌ}Œr¿?'⁴ßf÷?yÁ9®'ô?'⁴ßf÷?ï»àÑïÿà?p@qÚn'?Ët‰Ê?p@qÚn'AGN4FGL J1124.9+2143¿ëםy‰?@QgÙŽuyÀ;
)Ù]ëÀ<³ó;Ì_@r,…o7@B\=îx?ÆÝ«Â;#m?¥ùìj¡ßc?ã|楻æË?÷¼¿øÓç¿íxmÏç3€?ïú¬Î)Ä¿å{ ŠN£¿Ô	.3ð¿çnýäœÍ¿ÆjVJpKAGNbllSDSS J112503.64+214300.1?ïý¸Þ6	Z?&Ýý)êë?29
ŸÉ1(?&Ýý)êë?ïÙ샟?x¥ýÍm(?s	÷6@ ‡?x¥ýÍm(?ïçHã·?fU¾h!§?h·å´£(ð?fU¾h!§?ï ÿ&fF0?n¤cÀMqP?‡À6t,ãé?n¤cÀMqP?ïü)0ÐØJ?5 È›w`?>¶{6‹"?5 È›w`?ï:Nʵ½´?¢̈́qƒ?˜¶&®o³z?¢̈́qƒ?ïÕo†~<z?yê\$ý+?uH<®SßT?yê\$ý+?íÀ~òh+§? 3ên_?±ükâ»Ç? 3ên_AGN4FGL J1124.9+4934¿îri¼(²@Ož@ÈG,À:ыxn§À<5ÜF½S³@ò5#ù.€?øNŒ¥•P_?¹ÀÖIxD	?Ã-ÄßB›0@)ÃÂb@
'AÜCb?ålk˜ÕN|?ïÝ`='l¿ÍüÖö¿Õ]°ŸÅ'¬¿Ôbºõ8§¿å_ü?EöAGNbll3FGL J1124.9+4932GB6 J1124+4933?ïü¹N•º<?3'îò8"'?:5‹Ná³\?3'îò8"'?ïðš—:?`ö_aG?E?^ËÓUº‹?`ö_aG?E?ïÑ®/A¥×?x@ç>¦£?w(èl;˜­?x@ç>¦£?ïã§}ÄE?U›âȯUF?lX'š#5?U›âȯUF?ïöêõy5Ã?Lð6.WîC?R*LÍI?Lð6.WîC?ïÒJGdÈ?z¢2Rä,©?vÚ܃›ÏÙ?z¢2Rä,©?ïªQºTF¡?Š·ëšˆæ?…k'jîWÙ?Š·ëšˆæ?ïºzÛ?ruy¡#3?|8ýxï\?ruy¡#3AGN4FGL J1125.0-5804¿ìpBM,ƒ—@ ñ,'¦7À:M¼)çZÀ<zF"b@!þ"à$Œ?÷';ý?ÆûQš|m?Öw¦)ÊÔ¥@‡‰Fe?@K'à—ÚÓ¿ïýVlô!¿ï+Bn9™?ïýÀTïEž?Ð/ûZԷӿ͕c>"¹†¿ãϺ 9qAGNbcu3FGL J1125.1-58032MASS J11250388-5805404?ív~Ê?°Jk1ˆ?´OØË×±?°Jk1ˆ?ïb+:/?¢?š$a¹Lu?"º˜¿?u«?š$a¹Lu?í+8¬fG?¥Sì<-÷˜?¶§þ:œÍÅ?¥Sì<-÷˜?ï©é"ÈhS?uã!gίG?……šß÷.?uã!gίG?í.PÁ
§?°brï'?¶¥y÷'É?°brï'?êuYÜhm?ÌØÕƽáo?Æ*˜®^M?ÌØÕƽáo?ì½P 1`?©aGõV?º~þsõ?©aGõV?îdÖ`°€?¢ºۗT–?©¾2–…\?¢ºۗT–AGN4FGL J1125.1-2101?ål¡©]†ï@BÁˆ†aÀ9îÚøººÀ<:¿:=°@u,ŽSj`?ü©—"ÆÔe?¾OÓ@É¾?Ä÷'>]@Ôi
à"S@Þ跎ø¿ïòx6?ï>Áï#9¿Ò´ßñÙ¿ÝÑ·D¥¿ä¬;'}E¦¿Ýdæßr–ËAGNbll3FGL J1125.0-2101PMN J1125-2100?ïý_qŸ?1§{8,Ë?5u<cyÊ?1§{8,Ë?ïíúLjo?aÑXwcWt?bñÊòèw?aÑXwcWt?ïë¤Üe5?`W%=§\?d[îH¶'Ð?`W%=§\?ïϼ·'F?^Ü=¥t?x!¤WE0Á?^Ü=¥t?ïø[{O?J
é›túØ?N'zéñ?J
é›túØ?ﳒîÑü¯?‰ôL?4"?ƒDJ üJ?‰ôL?4"?ï¶m‰_(ž?…‡ž¼»?'dœ/6?…‡ž¼»?ïIj	S?"Þ$Þ½­N?–Ò½¥Þ
¡?"Þ$Þ½­NAGN4FGL J1125.5-3557?з¼Ý–t@7¾ÕϪ͟À9Ý¿zÔ²tÀ<:b'œOV@"A"ßÿ@ñÜPÎO?²ãÂË O?'B@c®Œ?ÒÄ«Á}œ@.~]Ë?ïÿ"g3¿áß
Q'™Ë¿à¬1¡¸¡ó¿â7´lƒ¶Ù¿Ùˆi[
lпßr&c$ÚAGNbll3FGL J1125.5-3558PMN J1125-3556?ïþvç×®í?úl¼?('†T?úl¼?ïô‰°©'Å?WÎbª>_f?VìžÛ—$Ó?WÎbª>_f?ïöËv¿¼?Môš2|¤?Rii?Xã?Môš2|¤?ïþ¶îf?GfêÒ±–?$žÓ;2?GfêÒ±–?ïþ#Í˶ˆ?&²['?-Ã%ÀÌ?&²['?ïÓyrÃÓ?{Ô3þõú?vCFƒùpƒ?{Ô3þõú?ïñ0Uœj?i2•î…)ƒ?]ŸUvÑ+û?i2•î…)ƒ?ïýî3é€Q?#u¶U?0Ža.	4?#u¶UAGN4FGL J1125.9-0742?á_xn@H¼ƒBÙÀ:"CïCÀ<_^4h½Y@ò¿ûƒ@ÖqáÄ«–?¿cÌ®…?`†K¤«?´É¼L!?öå§×ŸäŒ¿ïÌ7å?ï~•Òd¼B¿ã…Lò!¿â¾œ)¥ì¿ÙH¯œ:^¿á¥·]®1AGNbll3FGL J1125.8-07451RXS J112551.6-074219?ïúDNäi¢?@c¨…¸»ê?FîÃzB?@c¨…¸»ê?ïãi?u0<_Œ'?l–é­*Š‹?u0<_Œ'?ïÞÉ0ô·?q[€jܵS?p›áVX'?q[€jܵS?ïÊ⥸G?c ^þ×c?zŽ­+k™y?c ^þ×c?ïî•j9I?\Y-'m¤?ajê¿7?\Y-'m¤?ï'C‡q×f?•Í§¬ñ~ø?o&ùÂc?•Í§¬ñ~ø?ïЃÝçô"?}HjŒ<?w¾óH†´?}HjŒ<?îË¢ÖP§?•XÆ𳿇?£N…Õ.ª"?•XÆ𳿇AGN4FGL J1125.9+2005¿×âu´Í @QNµ ÝDÀ:ÁóTöÒÀ<m2ûÕÎÔ@ØdS爻@Âãú滋?¶h#ªÕM?«¬d!'¡Ù?ó¶îßFL@î[R×é?í.öWà'¦¿'ù†Fß,¿æôxþŸ3¿à2üâ>N¿æï¡ðÖ¿ïÿþÐñAGNfsrq3FGL J1125.9+20074C +20.25?ïþš¤? ­ÆGt£?.¦T1ÓñÆ? ­ÆGt£?ïök;Y¿±?X²ð^øŠø?S)ˆæÌ-è?X²ð^øŠø?ïçRH!W?tqmvr?ho­¶~Ñ?tqmvr?ïûZ&<)Ò?/oDã›Â7?B—fÊ ˆÝ?/oDã›Â7?ïý®÷¤¼¸?+¿þîÉÝÈ?2ˆCz¡•þ?+¿þîÉÝÈ?ïÛ®ˆÝ?ug%úu²v?r(û¢ÔP?ug%úu²v?ïÙJ9'¦i?€²³Œƒf?sZãÀO·?€²³Œƒf?ïöÇ.þM?CaM‰mˆ?Rq¢-¶b?CaM‰mˆAGN4FGL J1126.8-3829¿ê3\qH@5uX!)EtÀ9¥Ìô9ù À<>ô±d¡@÷oV¤ýP@|½ÀÀO?²Êà
œJÏ?¶˜ã¼'Ž@aÑü·v#@8³Ík-?Á4âö.ðÙ¿ÝEÓÿqá¿æs	¿àwy¥Œ¿ä3ZÖk®¿ïüev|^AGNbcu3FGL J1126.7-3834PKS 1124-382?ïüꐛÝÛ?)–•òñb_?8«|Îù܏?)–•òñb_?ïރer?x"ºþåÁð?p¾M(ù!?x"ºþåÁð?ïð¹x݉?bö=áÆYÅ?^
ÇwN?bö=áÆYÅ?ïÄ«@¾"®?`*òæÊ¡e?}ª_ªTÈ?`*òæÊ¡e?ïøøŒº«?@ڑÖó!?LÏz*3$?@ڑÖó!?ïy:Žœ:‰?–HiåǦ?Ø®/èJä?–HiåǦ?ïÎxMïw?wn©²g°?xÃÙ²Î?wn©²g°?¢€¯#?Œ¶—÷Æ8?¤eÕaXÑ?Œ¶—÷Æ8AGN4FGL J1127.0-1857?îã9bn¬}@Cɚ¿3‡À7s;dZ¬À;Y–¹‰$@vú«Ø5Œ@¼ô}þ•?"ÕÊCÒà?´ägH8¨é@!ŽGUÿç@ "ŒdQä¿Å`Ó)ˆ9 ¿Þožˆì£,¿ã‹à)÷¿ãèJ®kc¿æy2Pµ$:¿èžÎÂpRxAGNfsrq3FGL J1127.0-1857PKS 1124-186?ïøÖ5VN?G­;z÷?L§)®JR8?G­;z÷?ïçˆdèâØ?x,òK"W€?hw›$ۗñ?x,òK"W€?ïÞN5/À?xcŸ}9ä?pØøN
È?xcŸ}9ä?ïÿn:X?
±ÝEÎÙ??8·v³ú¯?
±ÝEÎÙ??ï÷D7<'<?GôBu|?Qw'½õFþ?GôBu|?ï\ç&H?¢NÂlõy?Œ(Æ8W6'?¢NÂlõy?ïàFakÞ?{ó£ÏË(a?oì¹[;Ê
?{ó£ÏË(a?ïþQ†§ÆÐ?$-O«¦Aâ?*ç"Qèï}?$-O«¦AâAGN4FGL J1127.4+5648?êRóÓw@Lbك"t—À:KÝþMxYÀ<ªþÊuÚx@
ÀaÖ	@mñf­´?¹A]˜a‹5?´ü‹+lÀH?õÈbŠ8ӆ@/Vôk!?ïÿäA2¥D¿è"d
ƒ ¿é3)Wèb¿êSi©¿æ€››ÒXþ¿ïÿþªJlAGNfsrqS4 1124+57?ïþ;8G?A7
K7A?,L|2Ùr?A7
K7A?ïøvÐ'0'?O8 gö_?N$À›S?O8 gö_?ïáÒAù#?sã1ÚïØ?n-¾=ãœd?sã1ÚïØ?ï÷î\¥®Œ?:ëë)eöE?P#G*õ?:ëë)eöE?ïÿ֗ž9?" ®FÓ"?…+>) ?" ®FÓ"?ïà÷SÞúL?r+œï]?o«ëkÌi?r+œï]?ï×8Z ?yÐh5e?tp}Ä6ˆK?yÐh5e?ïàÓ&Ö¦?^‰K×è‰?o,ò±Â?^‰K×è‰AGN4FGL J1127.6-4920?ï›wÃc @&Mv«XÀ:^ȋ­À<K€\±±¾@
P_=þ@@6m
J?Â_ý–™4?ÀÚÙÕÉˑ?úZë=Ñç@p
«T­¿å´d@q_>?ïû2¦Ey‡¿ç€"Töοâ¢+¾Ê«Š¿åÃà‡ÿå+OnÓrAGNbcuMRC 1125-490?ïû5˜"4P?=_!(n'?C)ðÁZM?=_!(n'?ïÈZ÷ñO?ƒ'²[?{Òù›d°f?ƒ'²[?ïé
Ÿã'?aÐɚCà?fõ`Gd?aÐɚCà?ïÑ7߯r?YÜôî–W?wd)$²Ù?YÜôî–W?ïã'yî?qiì¤vËó?lçnÃêìl?qiì¤vËó?î1wÝÃP]?µ¸
¸‰¬Ž?¬è'"ï*?µ¸
¸‰¬Ž?ïp'¯¾Ái?WU¬xÒ ?'û
¸6î?WU¬xÒ ?î¼PÖå³?'?ü¦þ?¤:ò'¤Ïû?'?ü¦þAGN4FGL J1127.8+3618¿ÓˆAºÏ8@Qƒk¹Œ~(À9m©PÇÀ<!gÝ^ëH@PÚqÐý´@в\Þþ(?¥·ÿʧÑ?¥õØ£‰vP?þ­üwµCC@侬ùrÈ?ë^Ɣ¤gS¿å®É¬†Ü(¿åøq–EQC¿â=fȋõl¿è"‹BhÛ6¿ïÿü¥¬¨AGNfsrq3FGL J1127.8+3618MG2 J112758+3620?ïý"½5øW?*Ö^á?3Ú¨3H€?*Ö^á?ïø
ÿXK'?P+%°=Ü~?OÈ'µ›b?P+%°=Ü~?ïèŠ*8¨?r×øk3o6?guî"ÎØÛ?r×øk3o6?ïú«éíï?7❻dfÜ?EPW¥Ù‰[?7❻dfÜ?ïüºŽç¡?3£RQ?:+¸Â3ê?3£RQ?ïÞ=ÆL?s —ú?pátÿMSù?s —ú?ïÓ͖£?{ÕG­Ü!J?v4¬G'´?{ÕG­Ü!J?ïö ²1?J"ëq†­â?R¿ÿ!>	?J"ëq†­âAGN4FGL J1128.0+5924¿ïÏVûöl@KU¬îàóËÀ9æ±iÀ<–[žŒG¡@ÎPV"œ@T¤°N?´ŸÈêTó?¶r:@SéG?ÿþÊuÚx@ªÂ»{싿ÒÐǘ°eŽ¿å¤ "ˆÞ`¿ä¤{(߿傚Nʓ¿ï¸Ê·H׿ïÿÿ" 5•AGNfsrq3FGL J1128.0+5921TXS 1125+596?ïü?>pÎ?0™ëûóu=?>Êu'M?0™ëûóu=?ïöáR8?S)•j]?R=ZèO¨h?S)•j]?ïáVž¿•¤?p@ ,ùcÖ?n©a'­,?p@ ,ùcÖ?ï÷Ëèîß?@éT+7—?Ph.gaë?@éT+7—?ïü¥8øÞ½?2ª[£?:Ö62äý?2ª[£?ïÞ=<mæÛ?r)ÇèJ q?páa°ObÇ?r)ÇèJ q?ïãWñ"¾?v­®Ó(bË?lè¨FÄÙ8?v­®Ó(bË?ïé_6Øj?ZYùz8®?fþ ŸìEÃ?ZYùz8®AGN4FGL J1128.8+3757?ïWŸ·üí7@Qd~¡ÆÀ9ψ*ÜLÀ<	óˆù8f@ÂQ} <6@?f"‹?¼ÚeÐÝ©?¼Fí¥4'i@£ÂÀ®@½Œ¾)q?©×•	'ú¿×®sûû8›¿åì§]§{¿á'Á(SÜ ¿ê²œÕŽ<n¿ã_gÍAGNbll3FGL J1129.0+3758NVSS J112903+375655?ïÝ2§t
?nÏÔ%s€?qf¬~?nÏÔ%s€?ïp'4*݂?"­‹%þæQ?'ï¹xìÇ?"­‹%þæQ?ïu©§6n?K²0n?'LJ',Q?K²0n?íåNC¸o%?'¾±ÑÕ½e?°Õà"¸Ø?'¾±ÑÕ½e?îaÕÅÄÅÂ?  eÞÓ ×?©â££³£Ü?  eÞÓ ×?íK"#|˜?½Þ 83?·m¦ïÀ>?½Þ 83?ílîÿ`?¥NƒD
c$?´˜ˆ
ÀØ?¥NƒD
c$?ãÉUõçž?³æ"f©Á?ØmT1îÃ?³æ"f©ÁAGN4FGL J1129.1+3703¿Þއ¨^,@Q€Ÿ¸fäÀ:<‹FðYÀ<`'o@á'C'¥.@ðäFfß?¿*^x[[p?´1 ‰Š?ö¾aßîé@"§×Êת¿ï ˆ!ö?âCbn_.¿ä›ª€qªg¿Þ³æ¡à¿æÔÎùÍ·¿çÁšÕü4AGNbll3FGL J1129.0+3705CRATES J112916+370317?ïþé JÁM?MC§D2?!eù™ê@;?MC§D2?ï÷4t"D?Qÿ~™Æ· ?Q–Å=Wk?Qÿ~™Æ· ?ïö}F
Æ?\.Ǔ§è?Sso«äì?\.Ǔ§è?ïøoe=œn?7%èKÜȍ?NBiùm:¨?7%èKÜȍ?ïþe›»1ð?#{ÑE(ò#?)¦A˜/Çþ?#{ÑE(ò#?ïÜÿ§aû•?tÝâ=á-Ë?q€,Zõo?tÝâ=á-Ë?ïòÎáúÜU?lýùëù-?Zb<€yæ?lýùëù-?ïæŽ0sª?],óñ«‰?iqϜÔO?],óñ«‰AGN4FGL J1129.2-1014¿ÔâÚÓÿ#À@GÑn¬†hÀ;9ÌýpÀ<¬Ök±ÿÂ@âŒXhvâ?ý²—a°õ?×5E2E?ÊQÈà5j?ò=0ýÎÍX@ÍîµÕº\¿ïâЯ°\T?ïgÂâ=Lg?éííÿL{Ú¿ÓVŒúk¿æ'4JŠgÍ¿ë#à¯Ø @AGNbcuNVSS J112912-101349?ïûRTǾ¬?5Jß-Ã?B¶¬
ê"?5Jß-Ã?ïê›Æ´H¶?eŠrW³âš?ed9ˆ0ik?eŠrW³âš?ïÛo?±yh?laŸÛ9»z?rH`*²è?laŸÛ9»z?ïµMä(Lê?i]Vù[(?'¬†î«Š?i]Vù[(?ïùvdš?C%<t ˜²?J&nÏBÍm?C%<t ˜²?ïÂù™ø‡?8ñµÜf?~ƒwÓÿü?8ñµÜf?ïÁËƁH?€ 
ÊÆ?ÊZ¾}?€ 
ÊÆ?ïN­aï?‡ÂN@@<$?–*Sڀf-?‡ÂN@@<$AGN4FGL J1129.2-0529¿´Ô!J•‰ñ@IçiüóÜÀ9¢š4Ê(À<$Sœ_G@;°É6@ÆX>…w?¶¦¢@²!Ñ?½2XíW\@sbb˧3@c¯˜	?ïzÇw"¿èhǍè¿ç"F{åS¬¿çhÁ?O÷¿ïÿülò¿ï³½œ®!AGNbcu2FGL J1129.0-0532NVSS J112914-052856?ïùîú&Õµ?Ej
{/T?HD€ƒÌ?Ej
{/T?ïïx–È6™?a©'2d7?`‡i7?a©'2d7?ïÊ´÷ß?O)=¥ú¾?z¥"'¦,c?O)=¥ú¾?ïÕÈI€Ã?`ÙÇxüHl?uۄžÖ\?`ÙÇxüHl?ïö6Ê䷝?PU3÷4`?S'j¡Ä–_?PU3÷4`?ïÁ­œ°ÐB?'Dת\C¨?)1¦çó?'Dת\C¨?ï•÷)'ý±?Œí\7¯÷?Š'5¯![¾?Œí\7¯÷?ï)ׂò	?‰U31\xº?šÅ¥J¸ò?‰U31\xºAGN4FGL J1129.5+3034¿çzcªŸP@Qð¼¾aÏÿÀ:¾ƒ""^ŸÀ<•È¥i±@«*"ýM@<§P;¶?Åׄᦣ˜?²Lêi?ë̘"¶ÛÊ@íØ>šð\¿Ý"±ð)É¿ç©¿+¤t¿ä£TY©¿âÅõåÊË¿ëýØ"kdÓ¿ïó ‰ƒœAGNbcu87GB 112657.9+305242?ïývs'aL?/¹|°ÇU?4Ld';ÉÞ?/¹|°ÇU?ïõ|,\‹?^,S;*"N?U§å*†?^,S;*"N?ï즞‡6?e«EÛë?cYaLÎsA?e«EÛë?ïô˜q+?@C±YÕv?VÏÞ-	ˆ?@C±YÕv?ïý…Fç9?17}~
‡g?3ÕÏåH'Ì?17}~
‡g?ïÙ;KZœ?v¯}]<¸?suâh!Á?v¯}]<¸?ïî2'pÒÈ?nüwÊèÍ.?aÍmUsÇô?nüwÊèÍ.?ïÉTí9¡.?gô<Ä&Ä?{U‰a¥?gô<Ä&ÄAGN4FGL J1129.8-1447?Ò¾P³ Ô6@Eє[l7aÀ9qÈÉ2
™À<ë˜iî±@,ZÝFA®@<bÿ©˜ë?²ýáÛ¹¥?ºWA°N'Þ@ƒ¶æ±za@
'õèO	¿Øƒ´?3°¿æ'Ž¿éŠ¼‡k ¿é+'Ëöä¿îC+κ㖿ï°ÿ|L¹AGNfsrq3FGL J1129.9-1446PKS 1127-14?ïýk.æâ?&v,2'î?4¦ˆW¯Žü?&v,2'î?ïôÕNyÎ?[AÆÆc×4?VUc×c2?[AÆÆc×4?ïâ]|Kľ?eÙËZSU	?m¢ƒÆ9˜?eÙËZSU	?ïÿ£Ùäbk>û"é|^??	vsӔ:>û"é|^??ïý%þþ^{?0÷ñ2±}?6АÌé?0÷ñ2±}?ïÑ­'ôÑ?|BZ³I×Ü?w)7û—?|BZ³I×Ü?ïÆÕàOi'?}*þæ5b½?|•á:h??}*þæ5b½?ïÿÀ«t?Ø'Ìs?gå'êäå?Ø'ÌsAGN4FGL J1129.8-4217¿Ð4r•k.@2˜ú7iÀ:Ç—×øzÀ<¯¦âWx@Å°ù³@"`št‹?ÉGHÿMR™?á|â(ԋ@öOv_Ù@'·þ¯¿î l¼Á¼Î?îPz×6³¿Ù·]d_%*¿ãä±i¿ð¿ïpêÄ.™AGNbll3FGL J1129.4-4215LEDA 566417?ìœQÌ?M?À$çô?»qž—¢?À$çô?ìa¤†÷D^?¼íÁ°?¼òÛÈEÝ
?¼íÁ°?åmzNG-?³î?+lì?ÕÙ%cq¦?³î?+lì?î·¢CC?Ž¾ªþ¤i?®"…á€Ð?Ž¾ªþ¤i?åîÂ3š¯?Ë÷F±Gé¬?Ô"{јʣ?Ë÷F±Gé¬?à‰ržÇŖ?Ò=Z´+–1?ÞíÂptÕ?Ò=Z´+–1?×AS-4Ò¬?´E.h‹>>?ä_Vie–ª?´E.h‹>>?åT÷àï?¶S·ˆf@?ÕV>!ßà?¶S·ˆf@MIXED4FGL J1130.5-7801¿ïXØy(_ñÀ/¨'ÿ'À9ÿ_,¶ApÀ<…I€|'@!Gø%ÁÃ?öŒ©[®|€?¾ ﹶÅy?ÅÀµ§Â&V@	‹)CÆ(n@RҵſÈp¬æR"Ý¿ïÿíáoq'?ïÿo¾ÁÇ¿˜ìû7昝¿Õ‰ yݒ¿ØÈ\ûƒ™}AGNbll3FGL J1130.7-7800SUMSS J113032-780105?ïí Œ½h+?d´
`£,?bßsNöm
?d´
`£,?ïì(€/mß?gÚª)ƒ¾?c׀ë¸S?gÚª)ƒ¾?ï×Õgâ"±?tñÇnn;«?tL?ûÆ?tñÇnn;«?ïâwÚé+c?VEº¹-?mˆ$Øû¤ê?VEº¹-?ïÖú¹«C ?rõéÕ´æq?t'£1퓺?rõéÕ´æq?ï±L¿²n8? ³àŸjþv?ƒ¬Ð|? ³àŸjþv?ïOĕ_'û?'øhóc?–m\¤Æž?'øhóc?ï°Ïï7?y…
"äë?ƒÌ Aû`Q?y…
"äëAGN4FGL J1130.5-3137?葽í@@<+-À;œ%¸÷,óÀ<ÆiH˜ö@#ÌP×H?õ~z#²Œ°?ѓa^j?µ|ã«`–n?Þ¢èB2›@e‹-m?ïךÈÙ"¿ítÎ6/g¿ïù–#?ïïšø>jŸ¿Ü®_¤U_¿=aƼàAGNbllNVSS J113046-313805?ïþˆÒÞ
? Ã"Ô<?
?'rΘůZ? Ã"Ô<?
?ïó2¿ÅÓ3?^™Uº9QÑ?Yš€íKØ|?^™Uº9QÑ?ïééT[»¬?h:¦gÔï?f«(‹Ü?h:¦gÔï?ïüJÜG>-?3w8n"m^?=©«{…ò?3w8n"m^?ïþVú…??%"6 Ì?*U	Ï{?%"6 Ì?ïÓÓpnÁÃ?v¦³v¥#í?vGé›^?v¦³v¥#í?ïæ:ÌQM?xдrÁÉ#?iÅ3'æ³)?xдrÁÉ#?ïñQ†'?]ž­a9?]Ýý€¯¡ó?]ž­a9AGN4FGL J1130.8+1016?éôBö'l´@P'»ƒÏ,ùÀ:e$Ã-çšÀ<b(Cëè@áðusu@Ëeè'?ÀÏa<0?¨?ž)\?âùâå=@s¦¸»ó·¿¾Ä(cvq÷¿çË@Fìù¿é%ØÝv¿èO‡A¨@ü¿ïâöý»'¿å§/^½O¬AGNbll3FGL J1132.8+10152MASS J11303636+1018245?ïôñ´ì9?PÅVq3?V•ëݜ?PÅVq3?ïëˍKq?g.K?âú§?dé4F¹Žá?g.K?âú§?ïÂãn=º?t‹9¡bÃö?~ŽHÇðÕ?t‹9¡bÃö?ïʿܤ[??f=Ò¸ú?z ÁÀš?f=Ò¸ú?ïÐ/´3ßè?|ƒú9,G?wè%çoä2?|ƒú9,G?Ëñ?"þgŸÂæ?Š½ÉÌ'»?"þgŸÂæ?ﱐÜ0Âë?ƒ$	9†6?ƒ›È÷>á?ƒ$	9†6?îi'|G¤?–œù2vîÌ?©cT9l¼?–œù2vîÌAGN4FGL J1131.0+3815?­¶Æŧ@@Qtw—|À9/ͶígÀ;Û£ûkq@‹D¤bË@d[Ëر?¬yð±ÙVs?ļ3b(¤@Š.Ýc@6c¿B ?íWZYè©¢¿äX·¼šO¢¿ç?³ÖhW¿è܀žöѿꦭj0ö¿ïÿî' ÇAGNfsrq3FGL J1131.4+3819B2 1128+38?ïÙM‰Ï?pr,$Ɠ?srÙKî8€?pr,$Ɠ?ïÜ}ܞÒ?|áx\[kN?qÁ•Ð?|áx\[kN?ïp0zØI"?ŒÏ™U³$?'ùð¨fi€?ŒÏ™U³$?ï©
ÚñË?pT³6•?…½IC?æ?pT³6•?ït²"7Ɂ?"&‡;8´S?'i»º¾Ù?"&‡;8´S?ï‹bPF]?"oLÎk± ?'køÎ<Ì?"oLÎk± ?í9X)ïP?¦vù]ì?¶5>°êÄ?¦vù]ì?í&Ž"½"v? Q§RïÚý?¶Ë‹ØɁÕ? Q§RïÚýAGN4FGL J1131.1-0944¿âˆºÂ;×Ð@H(A*2À:Ò
¨y0À<‹Cp˜@ ;øå¯r@"÷…zÿ?½µj/ž©#¿¨0€Á"Ö?î*käT¨Ï@u<Z#?ïϤMQÂj¿èZԂ"Úv¿â7}DÏ=¿àeòmpEã¿Ù˜,F¯çº¿Öç`Ÿý·AGNbcu1RXS J113104.6-094353?ïü~ÿm?1yšâî9??¼	O'>?1yšâî9?ïïä w?a®¿¡».?`éá°¾?a®¿¡».?ïôþԆÕ?Y'Mjñ?WÎro4ö?Y'Mjñ?ïñZùJÚ?A Ø,=—?]Jé~è?A Ø,=—?ïö[¯†Éf?HD'fþ6?SH¡v^3n?HD'fþ6?ïºßåX^ç?ƒzuÍ^Â?H¯°I?ƒzuÍ^Â?ïöž•+ö©?af|ÿŒ•?RÂÕÑMýô?af|ÿŒ•?廉©bº_?tl³Ç.É?†WU£áÌ,?tl³Ç.ÉAGN4FGL J1131.4+5809¿íϘ4¥à5@Kú¦">jÀ:}mÿ·Û¤À<²bÒ]/†@P1ÏZñ"@M••_?¼´È?œœà²'?âa…V¶K@þ•dU¿û¿ïqsªò‡q?ïõµú"pm¿æÇ1¢a‡¿ÑT‹<߄_¿ãí©¼&Œ¿ä½öp4E'AGNbll3FGL J1131.1+58101RXS J113117.8+580911?ïþ¨èþ?óûBC<–?%qnæLí*?óûBC<–?ïöß~ïãí?T81U%¶õ?RA¸Æ6?T81U%¶õ?ïø3Gց?;¡˜ÐJ—?O2à"ž´K?;¡˜ÐJ—?ïò÷9Þ|?BˆjOݖ|?ZóáyX7?BˆjOݖ|?ïýý{·[?&¿-¥‰µ?0"÷=2…?&¿-¥‰µ?ïÜ!÷ÕÑ?sÓIÖEA?qï5ÿg?sÓIÖEA?ïõä

\?_ҜŽyQ'?T7ê˜0Ù'?_ҜŽyQ'?ïØDAÎV?e
åÊQX?sÝß3¡¬?e
åÊQXAGN4FGL J1131.4-0504?×"ãøô"@J9Wÿ›V2À:¡›Æš"À<H­œ…Ý$@ˆsü|@¶ð<=ð?Ê-ë˕•(?ãØYÞBÀð@cì‰*¶@	ùBWC¿ìŒòãÕ¨?áœ#íEY¿æòŠêÕ¿êw»ûS¿è«ïxÉ??Æ­°½L§#AGNbcu3FGL J1131.9-0503PKS 1128-047?ïk¤ï
>'?™Oà"{?'‹b!Ç˽?™Oà"{?ížÛB©"?µG×Ù¨úÌ?³	'}|À`?µG×Ù¨úÌ?ì;"l·kð?¦Dû<	?¾#dšD ?¦Dû<	?îqwUïB:?˜J[ôÃ?¨èŠ¤{x[?˜J[ôÃ?ìôW˜öº?»r+';<¨?¸]C7U?»r+';<¨?ßàʦèó°?Òáîí‰÷?àš¬‹†(?Òáîí‰÷?å»zŠ4Ì»?´èójû‰i?ԉ
ë–f‰?´èójû‰i?Û/÷èý?¾2Õ.4	·?âhtž!?¾2Õ.4	·MIXED4FGL J1132.2-4736?î+"¯ÔÞ@*R¥'ÛçóÀ:&vŠ ØRÀ<K½¹3'Õ@ üSøû?ÿÌð©Jç…?µc+Ì¿J5ÖD¨x?–Ló½kI¿@"NÀ,€g?ïÿò(¦è7¿æ{B`Í 1¿ÞžáIå¿Þˆ£Ós¿ã3ªò‡qy¿ßÝ~ ÄÜAGNbcu3FGL J1132.0-4736SUMSS J113209-473856?ïü{Èð–£?2¿¬¬‡?<!¹û­?2¿¬¬‡?ïê.Ÿ1Ü?uûHí4?eÑ`ê­[¹?uûHí4?ïôâ_R˜K?U"Ó·Å¥ ?V;A~‹Zk?U"Ó·Å¥ ?ïò51î˜,?Em½ÌXì?[•œ_HÇ8?Em½ÌXì?ïüu˜Ì;?6öx|œhk?<S?z}.Î?6öx|œhk?ï"B=ïs?šz{\œ×õ?‹/p«Å³V?šz{\œ×õ?ïóúŸT)ß?hÈáA	Eà?X
Áej±Ý?hÈáA	Eà?ïގfñ·Ï?]ŒèUqP?p¸Ì~å'?]ŒèUqPAGN4FGL J1132.7+0034?íזr{P6@Lµb8Ú<!À8j¬=áÀ;ÎpmP@–Eý`@åM|Š•?ž±ç÷©"?™­ƒþŸ$??÷¹÷2ú(@	á þ'bÅ¿Ñ:b|vóý¿áX»]c³Y¿â¨B(ïb¿àíàBËV«¿ãÜU•:¿æµ£ñpwAGNbll3FGL J1132.7+0034PKS B1130+008?ïþ'Vüˆ?S)°‡q
?/6Ú¦4ø§?S)°‡q
?ïó}k™3Ì?`Юڤ ç?Y)>K—é?`Юڤ ç?ï褒#·?våq©N?g[mÄë‹6?våq©N?ïÞ,o®?b¹wÈÌ?péȝö?b¹wÈÌ?ïùÿÂ1W*?@M•­Ñ\ó?H÷ñ(1k?@M•­Ñ\ó?ï½;O6t?•®#þÝ¢$?€±,;©ð›?•®#þÝ¢$?ïÞo2N ?€. c¤ w?pÈfñ³ª?€. c¤ w?ïªóùXéH?}DMš7-O?…Cºó¹ÿ?}DMš7-OAGN4FGL J1133.8-2048¿ïòIÔ4u(@CA3 @|ÈÀ;J¥»æË|À<¬.î*§@ #áÜ~q?묔é0°¢?ä#²VÿÁ?í'I†\@¥#±µð?úÚ!nºË¿ë<…ÂL@?ïèq£±J¿æ­—}_§?ËHvü¶Ÿd¿çù_!£"ÿïúDÕ&§AGNbllNVSS J113350-204852?ïöV"ü?M"L{s
¨?SñRl¤8?M"L{s
¨?ïGxŒP'W?§%@•6Ä?—îr‹y ?§%@•6Ä?ï†ÌBÁÏ ?'Y'Ùd?ŽLïL›ê?'Y'Ùd?ï'ˆ®9å?ˆgÆ_bv?Ÿ
®ñûa?ˆgÆ_bv?ïÜç´Q"T?q+/¿zî?qŒ%ÀÁj0?q+/¿zî?íqîJÝ9?À[I"jýò?´p§`=?À[I"jýò?ï5e"L8Æ?'}AŸ1´?™S[±Q}=?'}AŸ1´?íî*¶É'?§!͕€¢€?°ŽªKoIw?§!͕€¢€AGN4FGL J1134.8-1729¿Âùéæě@DÔ€À;Wc$'†À<¢Y …F%@" Ӊ)‰ç?ôÁjî‹?ä),~ä®?ӂݕqì¬?üýî'ð2-?úkQ'n×ú¿ïƒŸâˆö´¿ëÓÂõ³uä?ïúgïÓb¿åfc á¡ñ?¬Dà"º^¿ÛUü wnÌAGNbll1RXS J113443.6-172853?ïú(.'?Awî_ œ?G]ÃfcÂh?Awî_ œ?ïëÀ`‹c©?i¤éìÕ?d?Ÿ¶"Ö)?i¤éìÕ?ï¤UF]È?}läwí3?†ê®uxñç?}läwí3?ïêLDÚ®?XZZ¤œC ?e³»•û®?XZZ¤œC ?ïø<Ä£ÕÕ?Pb&À¯Í?Oî-9¡^?Pb&À¯Í?ï¨Â9~"s?Í|#i?…Ïq£Î>?Í|#i?Äq^'?Š»ŸÐUÈ}?ØÎꇓu?Š»ŸÐUÈ}?ï°ÝßþÐ?Ô¶=¥».?ƒÈœ~ká?Ô¶=¥».AGN4FGL J1135.1+3014¿ïþSmwí@R@I<‰ô
À:ŒNrSÚsÀ<^6=@IϚ¦ã@ôQƜ1$?¿7)!Œlµ?†æՕ%õ?ËoY­€@_²ïyu?¼˜-žHÕÝ¿ä©Xž§ m¿æü­e(¿ß¦+xSδ¿àï€ô‡&¿ïø
ÞpAGNbllCRATES J113514+301001?ïþiyKú?¸ýïöÈ~?)nˆä2¡•?¸ýïöÈ~?ïøj÷^Š"?S)Պå8?NT!Êêò??S)Պå8?ï÷¬CŒ¿
?BOK†×ñ&?P§xsz?BOK†×ñ&?ïþ.xÛ«Y?´®ò^~å?-p~Æ¡?´®ò^~å?ïþ	É`f?#®h¤Ñ@?/cfy€"f?#®h¤Ñ@?ïÝÝ4'ȉ?yžUàA&Æ?qeÁš{?yžUàA&Æ?ïô҄
ªî?bß$nnz‹?VZø§¤°?bß$nnz‹?ïúÑJœ?7.Á
ré?EȺ/ˆì'?7.Á
réAGN4FGL J1135.7-0427?ï–Ã`E@JÀI¡3ÁÎÀ:Júì.'À<'cXK@4¥šõÿ@´£@ˆÊ?Êóˆù8e¢?ւc€Wÿ@<»r1v@p8²N¿âÉäà"Õ»¿ã²['ÕÝ¿çéüÞbvm¿êTÅ¿'Q§¿ß^?cR¿ïÿ‹Á>ÏAGNfsrqPMN J1135-0428?ïùŸj$G?C-+†:r?K¡'Fd>?C-+†:r?ïï¥ù4šø?aBÈÜ1?`Z¸'7 ?aBÈÜ1?ï~áu•?ƒÁcÈá_ž??£Ên$€?ƒÁcÈá_ž?ïîàwÆØc?H=s'yN?aˆ´Ï?H=s'yN?ïüVÂG?;­Ks€0?=O@ló?;­Ks€0?ï¬öÙ¬¸?"/Æ2$"ž?"ÂF%6?"/Æ2$"ž?î¢ÚǦ1?š $öi?¥ÒSSÉù?š $öi?ï0h¤?v?‹;ÈMÏ%I?™òëvYnH?‹;ÈMÏ%IAGN4FGL J1136.0-6824?çU;ù!áÊÀ3wÀ*ýÛÀ9ßzR÷À;Ý=ïí™@À¤[>•@7Á•aü?ÁÜæujeO?Æ9,œk@þ|Tå5@;BÄÕ?ïó˜H`Áâ¿Ð'¿ŒÈP¿åú!ßxËï¿èûYbFò¿Úa3ÁÎl	¿ðAGNbcu3FGL J1136.6-6826PKS 1133-681?ïá—¯tÅ?mý-µf§?nhÿp'£:?mý-µf§?ï ·_—?Û˝kÃð?‡øÒ$ª£:?Û˝kÃð?*oÈÃ?€èü¹:§þ?‰_uqÌ??€èü¹:§þ?XW¹?m×;#—2?‹—?48åÑ?m×;#—2?îÇm¿öûu? å>?³?£‰#ÿ´a¹? å>?³?íIHt/t?ºV¼Kž?µ·u»'`?ºV¼Kž?ë4vPƒ?°âÙ<-?Ã.&½ó¯Ô?°âÙ<-?ëî‡`m9P?¨µWUËeN?ÀEâ~KÂ?¨µWUËeNAGN4FGL J1136.2+3407¿ì˜Ä"Ò–@Rûüe@ÌÀ9犰ȊHÀ<}Mæ<à@¿8Ëùh6@ÝGËÂâ?µs[|T?¾w¾}~°à@.¾`"€@Ó×½k°Ó?ÖùXD¿ä´Ò9ô"¿æ{{*·å¿é%ãõ~z¿ç`…¡j€¿ïÿû}º@AGNfsrq3FGL J1136.4+3405MG2 J113627+3408?ïóâb¶-¤?˜Nâ5ƒ?X;:3o¨‹?˜Nâ5ƒ?ï÷™¾qY"?RP¹u;õ.?P̃_F:»?RP¹u;õ.?ï?VŸøt"?aLV
qʨ?VŸøt"?ïþCÄ>͊?'ˆ©,‰?+ø<0¿@?'ˆ©,‰?ïþ«Öªi?%^f–L®?&õ@݋xÿ?%^f–L®?ïÝììõ-¶?x›ÓîÇ£ä?q	‰£¥´¢?x›ÓîÇ£ä?ïÄrÇY³?}Ì¥(¦¹Ô?}Ɯ:Âvm?}Ì¥(¦¹Ô?ïûrü4ï?3qbyÏ?B7uú+ß?3qbyÏAGN4FGL J1136.3-0501?ì4¯ÙÄM@J‰¡ÎòAÀ:…0íÕ·À<³çcQ@Íe+'öê@º=c7ݽ?і]çM?Ýî~ƒÄ~@r+EþçÒ@'rÒZ€?ã'ZS<=¿âқ®FÏÈ¿æ̀÷Œ>¿é¦zÞB•ý¿ïÿÝe¡D‰?ïþXËs0yAGNbcuNVSS J113607-050156?ï®`Æ>hF?Ðíeð?"gÎiÞ¬¥?Ðíeð?ídºÐÝ?·Ë¯¾º‰€?³ôÚ'ÁI"?·Ë¯¾º‰€?íªY½"(?¡#roJ½?²¯3Ë,»?¡#roJ½?íÖ˜X?˜¼$W$†?±O/ZÒÂ?˜¼$W$†?î»z?Y?«¬Ÿ…ÁËg?®4H_~æq?«¬Ÿ…ÁËg?Û½…èÈç÷?ÑíA­°Ž?â!=›Œ?ÑíA­°Ž?è'"Û5_!?³ÍXt‰Šp?Ïaì"*ƒ{?³ÍXt‰Šp?ÙCh&§V?¿á+S•Ô=?ã^Kì¬T÷?¿á+S•Ô=MIXED4FGL J1136.4+6736?­p]úmU@Gú">iƒÀ9ÊÛ-¸ŸïÀ<Td«{Cm@ o@)»»?ûB%YUÜ«?¯bJßž? –´6þÄÂ?óišÐ@
"M'ëð?îŇ^-³?ÉO[¹¢¿áµR\Ä&¿Ô.ÁÙ©ª¿Ø1tí¿Ù«¨$v×ÎAGNbll3FGL J1136.6+6736RX J1136.5+6737?ïþݝmú?	Ý
†?"&0Ó¨­?	Ý
†?ïöáFLÚ?Süh½vø?R=×).»í?Süh½vø?ï÷ë¬`ñ‡?A
N¤‡?P(¦º+ñß?A
N¤‡?ïôru¾H%?AqW;'©?Wædv?AqW;'©?ïþb©J€?žF~ÄT?)ß11l˜n?žF~ÄT?ïے%9¨÷?sd<Cñ¡?r6íG®¤Ê?sd<Cñ¡?ïùޛV]/?^mÊ{ÁCæ?H…"0ˆ`¤?^mÊ{ÁCæ?ïíB·pÖ=?SvoÀ¦¨?b½H҂ƒ?SvoÀ¦¨AGN4FGL J1136.4+7009?ïùi$©$@FÒ·`,'À9¿¤EÀ<	?öå@x{‡µÁm?üÕýb–Î
?¢cŽ"u©X?yÁ"KùÕ?؛Øc-÷µ@
Ãsٖ‰Å?¤A_r>¿ØªÀ2Š—¿ÝžN¿Öš+¿Ù¦_$Ӟù¿à=At>–>¿ÁÃõãœrAGNbll3FGL J1136.6+7009Mkn 180?ïþ·0‹ì?û!"\¸Þ?$Œ÷£ 
?û!"\¸Þ?ï÷½»s?S8ã`?Pz"™—í"?S8ã`?ïõëÉ+{?a‹¦Ý¾þS?T(m²
?a‹¦Ý¾þS?ïøI›¡Ô?@Šä'H{¤?O¾Ù,ô?@Šä'H{¤?ïþscqa?"´[oLÓÈ?/xÊ?©=ü?"´[oLÓÈ?ïà؄³Oð?pê^N†*?o'{&4o»?pê^N†*?ïöw‰µ‡?f
ü½;C}?Sìsõ‡ä?f
ü½;C}?ïõ¬Ù§"?I>JǍ‹?T§üG1—{?I>JǍ‹AGN4FGL J1136.8+2550?ë é±¬WY@RQõ@‰]À:¯Q=à5_À<–/#ÙùÜ@ ;%Öÿ*Ã?ÿÇP ©Ã³?ºf¨UŸß¿£Ù,"=Š?êTø³¥@oZN€?ïôÜJ婭
å¿×Fb$S¿ã)ªžNµ¿Ü­ž^Ok£¿±!`ÍË$AGNbll3FGL J1136.9+2551RX J1136.8+2551?ïý ôäZ?(´ÃÊzL?6øWÿ–.È?(´ÃÊzL?ïõû]•»?UoÜ5½R?T	D?UoÜ5½R?ïò­2Âc×?h"h‰¦g?Z¥šp9'?h"h‰¦g?ïñE»S±6?A•
}k,Ã?]t‰¾R3?A•
}k,Ã?ïûE~Ö?Aùlk:à?Cþ듴Þ?Aùlk:à?ïÙàÉ%oÉ?w:äõÓû?s›K›ïë?w:äõÓû?ïù9(À"?\¤šÇ¨í?KÇLÜ£l?\¤šÇ¨í?ïÇo7Æ?ë?i"¼ ŒÒ^?|Hd–ž?i"¼ ŒÒ^AGN4FGL J1136.8-7413¿êgv±¸À(4¹#¢œxÀ9zŠ‡¿À;ã5ÍAfÓ@Äù·;–@%Қl'q?³z&P Õ?ÊËí>\\!@=s!_Ì@‹ú¶j	ß?ïýaŠ^"3¿Þ
üGä› ¿ã4ýØ"¿æ¦ãÏGÑP¿î:ò¥µ1¿ÑÇÒÝ2¸AGNbcu3FGL J1136.1-7411PKS 1133-739?â'àâY?˘6é²Fö?ÚÜ>;ÇMÔ?˘6é²Fö?ã×pÁM©?ʵò2ëmT?ØQ}eþ¯?ʵò2ëmT?æè?»=˜?±ÃH@Øښ?Ò/€‰…ØÐ?±ÃH@Øښ?é
}ìêÏl?¥qí+‡°H?ËÊLTÂO?¥qí+‡°H?šü!'.Ã? _&Ã<?ï/på¸? _&Ã<?¿X¨7ê?ÂòÞ?ì4êÿy?ÂòÞ?ÁÛK'?³'\#ŸõÝ?ë»É:­6@?³'\#ŸõÝ?Ťrt«gf?©`4'ŽŠ?ê–ãbÕ&&?©`4'ŽŠMIXED4FGL J1137.9-1708¿è²ÏUh<T@E"_ !¸À:–,Y$^"À<CõwæÁk@ ìç¢fé?õÂFçE?È(éè‹Ð?Ñs}\º@	£qÚ7ï[@)£šyhw?ÓP¯°\S¾¿ÞDÔÛ¹ú¿Îì%'›{?½e)$'"Í¿â6o]…í¿Ô?·¥ôïAGNbllNVSS J113755-171031?ïøS:‡ç?G "¨‰Ð€?N³,u¼?G "¨‰Ð€?ïëÙùÓc?j@ĕ—"œ?do&9Õ/?j@ĕ—"œ?ïÉNÐ?Š?zKÞ[ûá?{X—ëtzÍ?zKÞ[ûá?ïì1™Õ?Mºg¬Ø´–?cÎê-5»I?Mºg¬Ø´–?ïð¬NcK?]gèI½|º?^§b¸7¤?]gèI½|º?ï­	'>Ë1?'ïƜ¾?"½›~£Á?'ïƜ¾?ï˜
Ä
?ˆéMÉÒëw?‰ù}nt?ˆéMÉÒëw?ïÀ‡x@Ó?nHhH°Î?¼CÝæRÂ?nHhH°ÎAGN4FGL J1138.2+4115¿°*ÖVÒÝ@QXŠï²ªãÀ;`OËð.À<±§ðtqÂ@ 4C(ž¯®@,ZÑÝ®?½F‰§357¿¶dù(öC?û{
¢ò)@ÚD…ëçÅ?ëçlU"°L¿èùŠ—ž¿ãù.ŠWw¿åÛWª¿×ÙôhI¿Ý¯çä«:×AGNbll1FGL J1138.0+4109NVSS J113812+411353?ïþΈ8É?KƒžX [?.c -k?KƒžX [?ïô²Ì+Î?Vƒ£ät?VàšA,ß?Vƒ£ät?ïñä!¹Is?m;ö^EW?\7¼®©$?m;ö^EW?ïï6¥•ü?GGÁÊF»…?`É÷.o?GGÁÊF»…?ïüªG<?:)¼zæÄN??§zðØž?:)¼zæÄN?ïÏ·)ï´ü?vuç]G?x$jé9_?vuç]G?ïê T¹Ò?y"ìÌ;–P?e_úɂ½ü?y"ìÌ;–P?ïyŠÉÈ?':}rO%?ß®¡Ÿ"´?':}rO%AGN4FGL J1138.4+4857?ïÁG·¾a"@P†­-ËÀ:¬¸ô¨´À<¤k'QÕ@€šˆÕ@ÛçòÛ?Ào\¯-€¿¢3NSÙØ?áz‰hÉíõ?üâf´êØÑ¿ÙÚW¤×J¿ì`¯7¿Û¨üct¿ìåvã)Û¿ï÷³•Ä"?™A_(…AGNfsrq3FGL J1138.2+4905GB6 J1138+4858?ïóB%zŸ?Zîf"êt?Y{´ÿÕ?Zîf"êt?ïÙÂ3õ-?ÅhõúÒö?sæ%µ…?ÅhõúÒö?îâÞatº?–¢'ÏÖ?¡ÒéEì?–¢'ÏÖ?ï"eM…ð?yØSÜW!?Šæœº\óü?yØSÜW!?ïÔØ#d€€?x â…;)?u"îb]h?x â…;)?ïÚñ8ù?¨Í¦×
Ñ!?Ÿ¡ÐIÙé?¨Í¦×
Ñ!?ïV'^¥¸ó?ä*‰iÁ?•/´$i©­?ä*‰iÁ?뫐7MÒ¤?±Ó
Ä
áj?ÁQ¿"ȵo?±Ó
Ä
ájAGN4FGL J1139.0+4033¿ï""HC)@Qzµ^ñýßÀ:C¬­r"rÀ<4cʪ³@eMÌg@ŸžEÐÄ©?Átˆhî?µÚçÜr²?ñ¦+]{Ü@Á¿M2bÔ¿ëv_ß
¿ԕOó]ZN¿èƒ_›q
.¿ê"ö^ìtˆ¿ä˜íÂeÀ¤¿ðAGNbcuCRATES J113903+403303?ïÿ`~3Ñ?¡Ø§/«?Sêªd?¡Ø§/«?ï÷œÇÔóë?Qx•}¬.l?PÆoþ")Õ?Qx•}¬.l?ïáå<§‹?n¦Eµÿô?nÃLÝZ?n¦Eµÿô?ïüÞÚ¸À?$+
X5±}?9	(£'p?$+
X5±}?ïÿ›Ñ#Àò?ã«j¬ö-?	µçUç~?ã«j¬ö-?ïށÖ'A?s¢>hLmâ?p¿úÏC¾?s¢>hLmâ?ïÏLPæwn?~xÑE(
p?xY׫°Äð?~xÑE(
p?ïí'wÉn?Tÿ]H|'?bmècÊc?Tÿ]H|'AGN4FGL J1139.0+5530¿Éƒ²D¾Ôo@M_â?$ØýÀ;æéóN@ÖÀ=8C=lr@"ì¢$'–H?óÂ}qDç?Ög†aƒ}£?Î1·ÝýKÆ?öäí@	Û@gÿtißB?í!¼{¿ïÿð`OËð?ïú­EH­?™Ü8{$A¿•↦¿ÙsË©·AGNbllRX J1138.9+5530?ïúíw«ø?=uõ¶È´?GÀIäJD ?=uõ¶È´?ïõ¿ÌMë?VxÕoVÒ?T€g.èiÄ?VxÕoVÒ?ï×$wÀÐ?tÁ+ªbõ…?tmÄiRT?tÁ+ªbõ…?ïó e‹
?K~w¢'?Y¿5@›Ôò?K~w¢'?ïú­[ÔxN?E‡§=}"à?EJâµé?E‡§=}"à?ïà±Dk?o²³h?oN»ûrji?o²³h?ï൱l
?v"ô¼œ}K?oJN×KOb?v"ô¼œ}K?ïèÛÛªØ~?a°uA¸>›?g$$U''Y?a°uA¸>›AGN4FGL J1140.5+1528?ì̱8òÕ@Qu'·þ	À:þX;*xzÀ<†[3,}7@"«Hî†?ûŽîDì™?Ç#KŸÐ-?¢8¾Àù
?Ú'Â	Ð8@Õ̉…û,¿èÉN][$ê¿ïm"Ãqx?æ»ss•#¿å·¤ëàŽ¿"Ïюþ`¿ÓÏ-"óoNAGNbll3FGL J1140.4+1529NVSS J114023+152808?ïþ'^´7Í?¯=6?&ÚÇ"šI?¯=6?ïömš4†?Q·O
ÌÜ?S$Êژ30?Q·O
ÌÜ?ïîÖÄ6??[–¯ƒ·—?a);Ó_Ìæ?[–¯ƒ·—?ïø!æ?ö¡?A!ñôYj?Oxf8•Å¤?A!ñôYj?ïýb¹³•n?/†ÒÃöÒ?4ê1Jôo§?/†ÒÃöÒ?ïՓùدÀ?uô, žv?u6-Å'Â?uô, žv?ïîDàÉr¿?k\?a»ÿ"N?k\?ïæAöD•[?d'	Ä7É?i¾	É)¦?d'	Ä7ÉAGN4FGL J1141.4+6805?êÂI¡3ÁÎ@GÚ.	þ†ƒÀ:NjY¹À<Ž-ë˕•@ ÏU¢Hê«?öd»®²?Ãß\œc"?Ðñdûµ@èDŒ÷ʧ?ûº¤¦½ïd?ïåôñ¯e¿ï²¢´ËNH?Ž±ß¿È¼]¾ÍÖ¿âT,Ý®œ`¿Ïo¬ö˜£%AGNbcu3FGL J1141.2+68051RXS J114118.3+680433?ïnëyÏé|?—¾j.Ö?'"ÀÛf"?—¾j.Ö?í9©º¬—V?¼KB´©Þ?¶2²)QjÓ?¼KB´©Þ?îž_^ޚ?˜3(8'Êq?¦
^aj?˜3(8'Êq?ì™Ýf¢e?¡ÆÑ¡wþL?»1,ÊìÖ?¡ÆÑ¡wþL?î¦NùJ?¡Sr³o¼M?¥Ÿ›²®W?¡Sr³o¼M?å¼,õ	5?ӝz/­'ý?Õò‡¦í—?ӝz/­'ý?íІ{ëÄñ?¥K|ìiê?±{Ìê
|?¥K|ìiê?æ~_.Â=Û?¿ÜR€Y²?ÓA¢{"J?¿ÜR€Y²AGN4FGL J1141.5-1408¿ÙÀ«gˆ‹@F°Bž
A¢À:žë¥ÕçÿÀ<w»dg@ y‰®¿ñ?þãM­1üÒ?ÁBÎ[ÃO?¡p¡æð?á±ý2Æ&@
;"ÇOŠ¿ã7a–5¿ã,o_3l>¿Öf9ð¼–¿áòʍWkø¿Ûï½µ'®¿ß¤õî.FAGNbll3FGL J1141.6-1406NVSS J114141-140753?ïÿ-S
?×=•³ó°?U'aÝË?×=•³ó°?ïõ5bÒ!?Xð$šÝõ?U•:2'"?Xð$šÝõ?ïùéÖÑf?EÜn´H[‹?HX¤†ºP?EÜn´H[‹?ïþ™áƌŸ?j"øGŠ-?&aåDG ?j"øGŠ-?ïþø	¢?ʔÌyî¶? h)‹?ʔÌyî¶?ïÓ¿Í,e†?~µ­Ñ@Æ?v U߁?~µ­Ñ@Æ?ïûÀeéÇb?^˦GÚ	£?@þg¨i¼?^˦GÚ	£?ïüGƊŠÕ?0—°y@!?=ÁÉðŽë?0—°y@!AGN4FGL J1142.0+1548?ëŠv´oçL@Q"¿aª?À9˜€£ÿN)À<7€@,?ú@rŲ|>•@zãËìÓ?®pC£²û?†oHQaÛ?׏ó"
3`@ÅZ»g?קּ'›O¿ß¡D¾uñõ¿å`½§?õ¿áVÄ!Ølé¿ãÌ€ˆ¦'¿äŠšXz"AGNbll3FGL J1142.0+1546MG1 J114208+1547?ï÷:H ?BÝè"E©?Q‹n´AÔI?BÝè"E©?ïì[TÜȐ?pø,Õ{Ê?c¤ªóèz?pø,Õ{Ê?ïËõvå¸?z;Ø«ú°?zD¯$ÏÒ?z;Ø«ú°?ïŸDÒ©õ?vV&Ì¡D?ˆ.ËUº'Ù?vV&Ì¡D?ïÜ'Ôìg-?dTs\:ã?qìl?ś?dTs\:ã?ïÁu¯ô=Ä?ŒÞ»q6¢?E((=5ë?ŒÞ»q6¢?ï¥e`"#ð?ˆ|HB<z*?†¦§èõsö?ˆ|HB<z*?"Ž?–QZoõ÷¸?¥"ýÚz¤%?–QZoõ÷¸AGN4FGL J1143.1+6122?²ÀÄkÂUV@Jð² yLÀ:dIÄo0:À<"Ö"Üs3@±Fúæ:²?û͓fy±?Á9r½aÊË?ÐD¾ÂH@=À@ÍOª@xKôL!?ïñ­!5Ú­¿Ø´EíJ¿Ö˜"úUò¿×®«¤‰Ø¿è'I†[Ï4¿êÆ|†c[ðAGNbll3FGL J1143.0+6123GB6 J1143+6122?ïÞÆè…?p|bxò
?pœü"ü"?p|bxò
?ïò¦?'²½?^Vþx›9-?Z³ÓV
?^Vþx›9-?î³Úx'a?˜_''òÔ?¤ÂX{Rlð?˜_''òÔ?ïçÑݾ;?P°ãAî3è?h."ÑôÇ?P°ãAî3è?ïŠÜžÀ¹³?ڔJ"?HØZ g<?ڔJ"?ï¾æaÀ±®?ŸaŽŸÇYf?€Fg"ó"?ŸaŽŸÇYf?ëkðÍnC'?­ùqû­ÑX?ÂP<ÊFñ½?­ùqû­ÑX?ïºFø.qÐ?mÙ)³tåo?nAì|r?mÙ)³tåoAGN4FGL J1144.9+1937¿ïÿÁ2Ýn@RAÓØZÀ:byz?a?À<Íùóv…@y¬'˜ï%?ÿÑ!%µ¿?º'ú E?~qB"ãÒ?Å6½+o"?û½'(z?ïL¾õsµ¿ã¥óD/Û¿ÒñO‡¿àÒýž%ðU¿ã›šu%¿ÏB7]xêAGNrdg3FGL J1145.1+19353C 264?ïùýÏ#?>Y6ZO?HƒûãýY?>Y6ZO?ïðIŽ
è?aa]û;?^ýlÖ+Á?aa]û;?ïîán3S-?cáò"Mק?a'ôˆJ`?cáò"Mק?ï¦øXRÎ?nœ­þ\
0?†Aéݾ\~?nœ­þ\
0?ïóص–ØÓ?JÎ='|?XN"늣?JÎ='|?ïÃڗ)––?Œn€ýp¢?~´_†	?Œn€ýp¢?ïìfmû¹¨?r;¸î–œŸ?c™',!Ïé?r;¸î–œŸ?îÛý6?Æœa>8?¢Nà3˜"?Æœa>8AGN4FGL J1145.5-0340¿ïM{ì	©@K«#c²WÀ;¯ä	)tnÀ<ßæ Zé[@ ½'³K?ùÌ(bÙ?àèä?°8?à'õ|ï>è?ýƒîÑíž?ûîi_jÖ?ë.2x"P¿ïÿò(¦è7?ïÿVW$ª¿Ü^äq¯¿ãü°TDz¿ïÿÀäa>AGNbllRBS 1029?ïõ…v)°†?SH³Ï:L?TõöփS?SH³Ï:L?ï±$®Ç9v?‰!{*Ïé?ƒ¶ÔMÙ¬v?‰!{*Ïé?ï"Ã-^)x?¯î—è1Š?ŠÏ4²Äu×?¯î—è1Š?îÈdÇ0‹?Žn¥'«æ?£y³´ÅN?Žn¥'«æ?ïïääñ†À?hÖ[ߚ?`ÚW"?hÖ[ߚ?ï9-%ۏf?¡¡&µ.G'?˜Ú[BÖEE?¡¡&µ.G'?ïƒôœ¯?0åÄùk?Øê•Ê'?0åÄùk?í#°•éF?©Yö…FÀ?¶â{U
ôP?©Yö…FÀAGN4FGL J1145.5+4423?á_÷·\"@@QèÑQ­À;z8«B9À<ª"á{°{@ÇRÏ۟ù@oÅÀi<?» ¤iT'¿À*Ðù'7}@äpùg@.°',ä?ïŠ[…~¿ærùпãÓõ €"Ž¿ç
:'£¿âŽ7€ŸÍ¿ðAGNfsrq3FGL J1145.8+4425B3 1143+446A?ïý5$Ïî?.·Ïg‡?6V׌H?5?.·Ïg‡?ïØÁÑW\D?R–›"ˆÔ?sŸRò=?R–›"ˆÔ?ï戉>ä?k ë3Ù?iwwÜãû?k ë3Ù?ïнÅüV±?b
v÷N?w¡""?b
v÷N?ïú\ô¼nÊ?C'hÞ×?FŒ-Wbì?C'hÞ×?îó2ìÞ²u?©Ãøk©J? ÌÑ.¥<¸?©Ãøk©J?ïs±•¹»"?«ŒF†}?'‰ÍAécÄ?«ŒF†}?íÅ#Hj?¡L[i±j3?±×Žçvâ¯?¡L[i±j3AGN4FGL J1145.6+5552¿ëÛPPØé@Msb¯È°À;¼±AV¥À=	l«$™@çX"Öĝ@=m;l½˜?Ìþ0­ï?Kèü}ÉjQ?}âkÅuëj@70Ûê÷Û?ïˆ?Õ%¿ß"ä"'ï[¿Ø|Õ¾Ž¿çÀùYó']¿ÊòëÅ`qÛ¿ïÿÿ&¦³AGNbcu87GB 114248.3+560915?ïû·ÃGµ?=ÜY‹†h?C‰!±Vº?=ÜY‹†h?ï÷_Ö\÷?Pæ/'u ?Q@SÁÃæ<?Pæ/'u ?ïÆ?.éøW?ÂGym?|àhŒc¬Ÿ?ÂGym?ïû@ƒÂ‡?,h¸#"3?C¾þµÅë?,h¸#"3?ïöì¡å~±?P…:J×O??R&»ÚLïG?P…:J×O??ïàÝ)«?r¤6Êz3¹?oüáRðܯ?r¤6Êz3¹?ï Rúè'Ð?Šºa50*Ä?‡ëA;x(?Šºa50*Ä?ïé6î巑?Z¢ÆÕA.?fÉg÷o?Z¢ÆÕA.AGN4FGL J1145.7+0453?â"'¿}2@Og+©ÑöÀ:ìH£ÝÀ:À<t·×rB=@øW8ò@"{?;2?É\–#û¿³waì?çšr­™@ҘÛпÜބÛš¿é <€¹Îÿä†(¾e*ý¿íѾ¾í9?€ùu2˜?¿ïåﳁ¢,AGNfsrqPKS 1142+052?ïþÇÏɽ?-ŸÂõÄ:b?#ƒ?¾Ç?-ŸÂõÄ:b?ïóà‹à7R?bž§‹z?X>è)"Üõ?bž§‹z?GÕéÎ]?"v[ðq?€Ö
ÄÖÖ?"v[ðq?ïÿ2	^ðÉ?Ïáن™?¾ÎøIÿº?Ïáن™?ïþƒ²–Z?1FúnPU?(ÇÞÛ¼"?1FúnPU?ïË×ßü,?|]‹›Da?ziíà?|]‹›Da?ïÐr/&x?d'f#?wƸ9·Ü?d'f#?ïñMu(Ëü?Z,2¥ÿ	‰?]e'ZG)?Z,2¥ÿ	‰AGN4FGL J1145.7-6949¿ÙW ÈJ~À»?l&šÀ9èn"2QŒÀ;Ä]¨QÃA@c6æÆóð@S'ˆ?ŪD'?Ìûúâ´À'@é¨ÛUüŒ@\\¥t?î¶ãâ.V¿çÜ¢˜E܃¿è›¬>ÿ=¿î$Ä:Wã¿Û7ã¼R,¿ïñâ0`†AGNfsrqPKS 1143-696?ïüškŒÒ?5!kbp¿k?;,¢`ó?5!kbp¿k?ïéÆBD;?n5Ü\?"?f9½šæ"ß?n5Ü\?"?ï«jš†1;?z*<'BK?…%YME¥s?z*<'BK?ïð~Àº?F6'y°œ?_Ô…Ív?F6'y°œ?ïûG¨;?Cn ¢µÛ?Bãݔꝩ?Cn ¢µÛ?ïqbÔWþ?Ÿ'úßqÐ?'Ü"®7?Ÿ'úßqÐ?î@i¾¤YÖ?Ðøä)v ?«ùdr0¡?Ðøä)v ?ïC¸kcGÅ?‰5†"-!W?—ˆòŒ·Ï^?‰5†"-!WAGN4FGL J1146.4-3327?ˊ@~RôÍ@;zãâ"À:æÄ©Ü¡À<€ëaŠR@26ï©@íàBËV«?Ïڿԗ?ÒmõJ‰;@;ç+y+?õÑÊWÒyà?ïõ/¢/k?´€îýÏ#>¿åÞ¾Ò8F˜¿äè)UJµ¿ïñp»Sþ…¿ïÿÿ)@k*AGNbcuPKS 1143-331?ïœZÓyþã?‹lå«¿?ˆéK(_?‹lå«¿?éƒ~Ç}¤é?°T¶.·?Éòâ	l]?°T¶.·?îŽf	Ê.7?'å!ß!-å?§Ÿa¥N"?'å!ß!-å?ê(.ÉÛÅ}?£<h
1ZŒ?Ç_Dؐê?£<h
1ZŒ?ï" 2ÇÊÒ?–jN¹‡±Ì?›»ù 'mÑ?–jN¹‡±Ì?ӐâÉÁÞ?ÍÏ €i`?æ7Ž›ù?ÍÏ €i`?ëÚNQéùü?¨¦š'uµz?À–ƸX?¨¦š'uµz?ÓˆáC/?±Wm1–+ú?æu;^h|?±Wm1–+úMIXED4FGL J1146.6-2902¿íÄiÀ@?¹Áç–|¯À:ãòènÀ<Œ°"‡áá@_ʇù@<'Éä»?̟á²7Q?ь!f,/@부#§@†)ç0'?ä1£{š«?îúÁ'›ü¿ålÉVö†Ú¿è´Zåÿ¤¿á˜'Bdÿ¿ïûM³çùyAGNfsrqPKS 1143-287?ïïªfÌ?XK·˜nš?`U™Ä¤W?XK·˜nš?ï¬jö²¾?Œá?ï†?"åBE'ë?Œá?ï†?ï¢TíÜ֟?{ç…pþÖñ?‡jÄwœLZ?{ç…pþÖñ?ï‰óÁ$ÅT?rç³uá'?ƒ©;)?rç³uá'?ïЬ§,C?s{F!>j|?wž©º(Na?s{F!>j|?î'ƍ†Ä?°'8½"Üþ?§ÓŸÄ"Þ¾?°'8½"Üþ?îå:èðU?¢=‡ÉË?¯¡¬U¼}¨?¢=‡ÉË?ìä—	؂?£íÂÑ nŠ?¸ÛG³a°Ž?£íÂÑ nŠAGN4FGL J1146.9+3958¿'ß«ÎYÒ @QÝ÷'j@À7À¼O§@À;ŸÝkí@ådÉ-[@"ÚZT	m?"Mé=Ï?±/à~–š@ɝæ?@ZĨ»ö¿³ÊÅáv'$¿âáT¾É(þ¿æHmWoÈ¿å'pjÌ&µ¿ç½jΪó¿éÌò!+ûAGNfsrq3FGL J1146.8+3958S4 1144+40?ïûΘE ?@´¶Hƒ?@Çü¥T°?@´¶Hƒ?ïóo{êå?a1ÙY¶ŸK?Y!Žóç?a1ÙY¶ŸK?ïëŸTˆ\I?gÍwµ¼6?d`«JHÞù?gÍwµ¼6?ïþ,,üé?!)Ú_u?-=4Dåý¥?!)Ú_u?ïýòÉw`?1Òۚž?0o	3 jE?1Òۚž?ï¹/ïå^G?˜–ÅY
ù?´˜ªT?˜–ÅY
ù?ïë‡\P?sBË&èuÂ?dx£æà°k?sBË&èuÂ?ïúÁÎÛ´‹?=‡ùa2™?DøÄöâC…?=‡ùa2™AGN4FGL J1147.0-3812?ïA®fkÊ@6ô	å\ËÀ8v`' ×À;±d¾ÆyÌ@là{U`Û@G
=p£×? Î»do–;?«ð~ã"õ@.®@ð‹@½áÓo(W¿Å*F$§5¿àÙ§'æø¿ä‰¤úì/¿àõo]°à2¿è¬übf§¿àÍ7¡AGNbll3FGL J1147.0-3811PKS 1144-379?ïý(.Ù?2R`uïvÊ?6»Æ
MŒ?2R`uïvÊ?ïï+?eH3uÐH!?`ëôþ—¼Ÿ?eH3uÐH!?ïá¨5,¡b?sYPž"h?nWʒÅõÚ?sYPž"h?ïú"¹ô¿?2ª5"4J?Eícp­R?2ª5"4J?ïú³\ZÁ9?BzE#|n?E2ŽÞ¥î"?BzE#|n?ï«Ü@¡õw?™.4L·'?…ïåA
?™.4L·'?ï«hm46?‡#CQ
Ž´?…%ùë'*}?‡#CQ
Ž´?ïïïғéµ?R¼-o[Kæ?`-(½óp?R¼-o[KæAGN4FGL J1147.2-2627¿íØ2"œ@A\1YÀ:
'@ßÄ À<T·«c@2—"@÷$œ—zÛ?¼]v}µ¸^?»´jÀ¾ ¸?ù]RV)Ž@ìéõýr²¿à'#€Õ¦¿ã{V'Ô?¿èÆB¤À>I¿å'EØQeM¿ëۙN?F¿ïíœtÜAGNbcuPMN J1147-2625?ïý/'X¡q?2ÊÚUDfY?6ƒlәÕn?2ÊÚUDfY?ïôzØçb?WúΛ®C?WðVpKV?WúΛ®C?ïç©Ý^•b?o\¢${$?hV"…í¾€?o\¢${$?ïý¶	os? (H/¸Áè?2O¶'"#
? (H/¸Áè?ïüô³NT*?2&aàèû?8ZcØÝ#&?2&aàèû?ïÏ[v.–¨?~"F™ìù‡?xRDó€.?~"F™ìù‡?ïã3{­uo?x‡¶îC?l̄Šä)?x‡¶îC?ï÷ˆëª=?AwžQà¿"?Pî(…cæ\?AwžQà¿"AGN4FGL J1147.4-6758¿·þu$§üŸÀhaýKÚÀ:I:MÙ§§À;Ë
ù½Ç@_‹p¶÷M@§ø-ýi?Ì@x@-˜?ٿώH,¿@žÈ~‰rÛ@uœ9\¿Ùçwþ"E¿ãRôÏJU¿åD(Müã¿ê­x:¤A¿ïþûž‰s¿ãlqãr*ÀAGNfsrqPKS 1145-676?êJgF$x?ÀÒ@¦Ó?ÆÖbçoª!?ÀÒ@¦Ó?é7|&Ö8?§÷oZ"?Ë"g"§"?§÷oZ"?ë3JMè&?ª!Àq¯ ¾?Ã2ÖÈ_eý?ª!Àq¯ ¾?ìÄ"6x?˜ÃÕ­FÈ?¹ß[g&L<?˜ÃÕ­FÈ?ØåGNhv?DŽò%É?ã\rØËÅ?DŽò%É?Ǟ2£žÞ±?É®<b'?êsWHT?É®<b'?Ѧè.˜¿?µB·A—œa?ç,‹èð³¡?µB·A—œa?Î^p<—ϯ?³—LÓ¼?èhcðÚ?³—LÓ¼MIXED4FGL J1147.8-0724?ï'L£œ§Á@JßeUÅÀ9yæ'æÀ<TTëêŸ@d"ZD[@¯¸õs~?±òù²3†?Åä=;IØ@Ø\$ħ@~¹*³?ïÚua«ì'¿Ùº·Á¢Í¿çêßÂrÖ·¿ç_XŠÛµ¿æ…Lp¿ïõæÁÀ7AGNfsrq3FGL J1147.8-0725PKS 1145-071?ïöÄŒéï?IݍxÐò?RwÄ´±Â??IݍxÐò?ïóІ›?_Eߏÿù?YÒ_o¼zi?_Eߏÿù?ïÃvðŒ^?s
Ë tû?~Döˆi¼Î?s
Ë tû?ïúnÄü?1´@õú©»?E¾D)ëÐ?1´@õú©»?ïö^§¼XG?PY¨s#?SB°JÖS?PY¨s#?ïÀ^,04¦?ƒ"©<Ë
?Ðé÷ôÙ?ƒ"©<Ë
?îÄöÓlµF?—`c–H'?£°'ÈXĞ?—`c–H'?ïë|ñð?Rz-hÑú+?dƒüîoÊ?Rz-hÑú+AGN4FGL J1148.5+2629¿Á0øùÙþÂ@RýàŠï²«À:–°ä+ŽÀ<oÅµW@£I.G;(@§±9ÉOj?ɞ¥2?¼HÛæñN?îõù`½°@¹î£·*¿ÛBž54À¿æ;T»,¿ëSà4éí¿èvk—'ÏR¿ïÿ³©æ÷¿ïÿè+ÍäAGNfsrqTXS 1145+268?ïü¡ƒÈÌã?3ºæšû?:óâ^†'Š?3ºæšû?ïøvËR=(?PÏyßÏ?N$қÁ¡?PÏyßÏ?ïÞ$Ѥ* ?oہ[5a?pí—BˆX?oہ[5a?ïú7Iÿc´?2#•Î4^2?G"×a]"?2#•Î4^2?ïý|uŠö?9$Ï'lŸ?4X2#(ä?9$Ï'lŸ?ïÖ.݅y?{º•wÖè8?tè'G1a?{º•wÖè8?ïã)lØ<å?rYIù»?l֒ôèãl?rYIù»?ïÝE")Öú?bM%š¿Ä‡?q]=èTÒê?bM%š¿Ä‡AGN4FGL J1148.6+1841?ؕRÓó˜Ð@RQ'U°5½À:œ2ƒ
À<'HÌ!¬"@ÚÏE"@7›x¦?Äuƒ9ÛÃá?§e"ÏãÙ?ãO؅g³n@Æð)s@ê?ìô´!Û¿ê&$V÷]š¿ãÃQùÇכ¿×$:ýöe¿é Ÿ>À¿ï÷,ÊxAGNbllTXS 1146+189?ïüÿGHhú?,³PÁ
ç?8Åù1LY?,³PÁ
ç?ïöâš)?VPõŒÆ¹Ä?Sæ:Éýò?VPõŒÆ¹Ä?ïîH1"o?faªôÆ ?a·ÎN´Ck?faªôÆ ?ïõ3P‹??I'¸FÝÜ?Uñ˜ä0úE??I'¸FÝÜ?ïùÙat}ð?>ރkð@?HšyxœàÕ?>ރkð@?ïՅÞPض?{B‰î#L?u=ÇÅqO?{B‰î#L?ïàð—Ï?x½¥'aÅ?oþØj°½?x½¥'aÅ?ïݺ€øk•?\ðÓ;¢ª§?q"¿|;´?\ðÓ;¢ª§AGN4FGL J1149.0+5924?ډY?·P@Kû`¿]xÀ:¼¬'\fÀ<—ˆü"cõ@S*¡iFÁ?ýØPXÝç§?ÑC¢A2û*?ÍwV	L?ö<py@œúåcǿᲈˆ˜À¿éu0™$ÿ"¿Ô£"ŸXö¿à—¢H"Ä¿ã…WWÕ©ë¿ðAGNrdgNGC 3894?ï÷¤-`$G?CšQFËo?P·¤Ôƒ¢ÿ?CšQFËo?ïóy¦[ý?VÇZÊ__æ?Y
Œs?VÇZÊ__æ?ïÜ}ŠÖnr?gJ7H!?qÁ:ŠyòÞ?gJ7H!?ïɆïüZb?^¢ý{*j¥?{<ˆPï?^¢ý{*j¥?ïôâcªå?R'VsdÀ?V;:#T¸?R'VsdÀ?ïÐ3¼-?wéµ»z?wærN,?wéµ»z?ï™k$Õç?ˆ|ȎµÌ?‰¥6ÍõÖV?ˆ|ȎµÌ?ï1>|ùŒ?ÆØÉߢ\?™Ø0_±Š?ÆØÉߢ\AGN4FGL J1149.1+2819¿ïµûx(R@S
†½ôµÀ;5º>TÏeÀ<¹šTbX@îÎxžwO?ú:73rô?ە̅0b?ЮrĘ Ë?ã ýy¼…@œVUi?첁Çë¼|¿í–ðÝMM'¿Ü¶¡gP¿Òòœ"%¿ä°Ëæ¿ïýYÝl[AGNbcu3FGL J1149.1+28157C 1146+2841?ïýzh??%Ø&"à°k?4,¿w‹ê?%Ø&"à°k?ïöZ¥=Ø?XPÚ¶Så?SJµüà5?XPÚ¶Så?ïà'þéj?p2€H£Q?o}҆-?p2€H£Q?ï÷CþSúË?5ÉÔ*‡?Qxï–IÝ?5ÉÔ*‡?ïþ4¹Î ë?&ïry=¡?,´gR¤?&ïry=¡?ïژÜý"á?yÎìÜ?r³'"§9?yÎìÜ?ïæ5á8j?r9›Ö­o¾?iåÉꍆ ?r9›Ö­o¾?ïïÖíb¤?K®ý[Ù ?`)á?³½?K®ý[Ù AGN4FGL J1149.2+6246¿í'"÷©¢Ú@Juü–þµÀ;C`dÄ¥·À<➽ÅÈÍ@î]ìn@åRº·÷S?Ä(2y$?¿¬'Ó|"P/?啬¿ç<?üUŽ¿öЁ¿âVà±09¿á?-!¡:x¿áOÝO³¿ããY '¬m¿áVó+Ü'¿ïÿÿ)@k*AGNbllNVSS J114926+624333?ïú¢Q½Ñ¡?A¢{Éį?Ev¸®&µ?A¢{Éį?ïî*#%Z>?iù)'ñõ?aÕܘ­B'?iù)'ñõ?ïÕ­lÆc?r†åæ7ý©?u)IŸŽ)¿?r†åæ7ý©?ïÛ4|?VhZ?reÂV†?VhZ?ïõ'!ïد?M)üÙ 4'?TÛ¼Žñt?M)üÙ 4'?ﯔdÛÀ?‡ŸÇF€5þ?"æÔiˆ?‡ŸÇF€5þ?﮳žÊÓE?ƒ#Ò[™¼$?"S]qX³?ƒ#Ò[™¼$?î»û˵B?''<^>Êw?¤@CBô!?''<^>ÊwAGN4FGL J1149.4+2441?ì	Êó?
˜@R÷l7`¿]À:îY_æÌÀ<
ª}íl@ ÉêWÍ|?ýz¬(©l?ÎՑ—l™?Äk«õ'½?ùƒX´Ï?ú^/5L¾¿ê{`"¾ŽF¿èç6žË2¿àÖ|x÷c¿Ø]]¾¢¸¿äå}ºŠ¿Ò^(_ÀñAGNbll3FGL J1149.5+2443RX J1149.5+2439?ïüŸÊû?aÕ]!룂?;sg¨n?aÕ]!룂?ïÎ>Yüo?ƒ™Ç¬ô_¤?xàÓ-Ó¼š?ƒ™Ç¬ô_¤?ïêG
Ê^?`öíéò1i?e¸pûAç?`öíéò1i?ïŒÀ«tD?sLÆcÛ?ŒÏÕ9·?sLÆcÛ?ïû³ÿ?7æZ­.?A/ÿ7S"ª?7æZ­.?î»eC-…?±8ùDÍk?¤I«Ï	³?±8ùDÍk?ïà9ˆ"?ã?qÖ¾£I\Ê?oÆw7íÏ?qÖ¾£I\Ê?ìx›Ìh'ª?¨hŠEþ6Þ?¼;!œ»j­?¨hŠEþ6ÞAGN4FGL J1149.5-4029?Ê7=ïN×Ô@4Þf˜»MIÀ:(3û°À<;šß÷.@-' %ú»@lŠÅÁ@?¼†êªÙ2?ÀbHIšÓ«@ÑÄ2ÊW¨@
®"ѶkŒ?í€ÿ90£6¿ÅG³Gë|¿åÓ áŒwr¿ç'
~ß0¿â9ã¡$¨V¿ïÿþó…õAGNbcuPMN J1149-4029?ïý´¸{S?(Ï("øE?4Y}î8=?(Ï("øE?ïí}5N°+?c¼Š¦‰Ü€?b'ÊÒL¸?c¼Š¦‰Ü€?ïêc,Žî	?b7³m¦±»?eœÓo²6?b7³m¦±»?ïí^ÝÛèÊ?E%܈8?b¡"xN‹?E%܈8?ï÷RûX.?N
J6¨O?QZ	ӔÅP?N
J6¨O?ïŸbá*¼?ÇþÁq?ˆ'GdzÁ
?ÇþÁq?ï¿,ü€l?€¼ëJ"¸Y?€4Àë±Ù?€¼ëJ"¸Y?ïªêõàJ?oâ›9¥‹?…EB'<QA?oâ›9¥‹AGN4FGL J1150.4+2418?ÔnXdèYh@Rþ€sWæqÀ8Ý^žšÀ;ÿ…ÄÐ	@
;ƒcÍ/@Š82vtÑ?¤ð?éØ?­‹ÊNe!@Ñ™Sù|@
H¿ "_ž?éT¯àÄ¿à
RÎÙí¿äF¼x{¿áº(»
,ª¿æ¤Ùžlg1¿ì~õ†÷AGNbll3FGL J1150.3+2417OM 280?ïþšN0¡?œ"ŸH?/FX°ÖÈ?œ"ŸH?ïê÷	º?hb"?eëü6‹?hb"?ïíZ7O~?rv	7ßYà?b¥È¼õÑÂ?rv	7ßYà?ïvËØ[ ?}¤SîQõF?',Fƒ<Íö?}¤SîQõF?ïü
Šûú•?4ëéIRóF??«©«-3?4ëéIRóF?ï¾>êv€æ?'ò6æ²V?€pEsÒw?'ò6æ²V?ïÜyuŒÉý?x·=†'Âf?qÃE#l?x·=†'Âf?î6'•h?Ÿæ=¸ÒÞ?®¬—ØaF?Ÿæ=¸ÒÞAGN4FGL J1150.6+4154¿Û'££@Q«øʁ˜òÀ8²¶d«{CÀ;š‹'!­@"³<Î?ùæ)_tڝ?¨î´Âٝ¯?º?©ƒ	@ãá!îgQ@§‰§´¿Â¢£C â¿ÓvÍ;Ý{Ç¿Ö+P%\Zõ¿ÔjzýÍÙ¿Ü-þ`BµÝ¿ä&œˆŒAGNbll3FGL J1150.5+4155RBS 1040?ïøÏ>cŠ`?KèÁð±Ë˜?LÃ_>?KèÁð±Ë˜?ïéàú‰Ò?u]?0Ïy"?faT&?u]?0Ïy"?ïԁpF ?yóagH@?u¿xGܯæ?yóagH@?ïÝüw+Òä?Vî0yWð?qÄif¡ü?Vî0yWð?ïð‹ÿ¹D?avÒeW8œ?_Üèc'6¡?avÒeW8œ?ï°XšBXb?"UèB]Ãa?ƒéÙx°Ù?"UèB]Ãa?ïÙ¯¶"?'=ÉH/s?s(@s‰Å?'=ÉH/s?ï{<GµÉ?yÄ ÁFªá?˜wªÞ?yÄ ÁFªáAGN4FGL J1150.6-4823¿ì¦•åsÑx@*…ê̒jÀ:,Ù=—ÀÀ<Uäßq@ZT4_®@ÕM¾Ñb?ėܕ—¬Z?铙¥X½@V́Mrz@uOVTux?ïýý'¶œ¿ÅŽ"½"u˜¿è6u¨"ÉY¿ïÿ°NçÄ ¿Öÿïcû}?ïôlj£'AGNbcu3FGL J1150.7-4816PKS 1149-480?ÅÕMNN?Ê VߓW?ꊠ ,¬m?Ê VߓW?Î'5Än?ɵ€U¾?è{[rŽà%?ɵ€U¾?â.
Ò
u×?µM"_,†'?Û£ê[åS?µM"_,†'?巚Ã\­ø?½è#fЬ?ԐÊyF¤?½è#fЬ?Ðêq6è¹+?ÎÁ~¡+ðZ?çŠÇd‹£j?ÎÁ~¡+ðZ?"¡§®O÷?žÄ_í'?ï\òù‡@?žÄ_í'?ÞWßs\?Ã
‹¦3?àýÔrFR?Ã
‹¦3?«üÒÒ_Ñ?«¬×2-.?î@2Ó	"?«¬×2-.MIXED4FGL J1151.3+0957¿ïcÔ/[|@Pï‡~äâmÀ9î{Üð0À<^RèÛ M@Xx]Öu@9^á6ç?³ê©ó¿ÇuçY?Ùæg¨…ŧ?ûáHÒ©¿å")uš¿â¢âƒw¿ç9iãÉh"¿ß?üoQÇs¿éa[?êx¿âðŸdß©AGNbcu3FGL J1151.5+0957NVSS J115117+095826?ïò‹®}	?VœcçÈ´	?Zè£ì"t?VœcçÈ´	?ïæ·[Ä?qƒ¶Ð®{?iH¤`ü?qƒ¶Ð®{?ïªÈ2*Áí?'G4Ò܏š?…Móƒ
ô²?'G4Ò܏š?﬋Å%}?rYø!Ÿö?"Ý>Ç×h´?rYø!Ÿö?ï¢g'-¨?|ô¢"k¸?‡f?½Î?|ô¢"k¸?ï…r9û›º?"Ï]#[I´?Ž£q"ˆ­'?"Ï]#[I´?ï)"Ό¡?"YfÒÁ—?šÛ¦'ž3ð?"YfÒÁ—?íýG¬š…Û?¡EGÞð?°œ¸$?¡EGÞðAGN4FGL J1151.5-1347?Õ;bFœª@GIÿ¼ä!À:+oðSÀ<L•¿ðEx@Fs´N?þ¿4"…ƒb?·ŒÍ|²?°s¿jc¡?ø õäKj@´~wTJZ¿åVÛó[¿Ÿ'gB¦»
¿á×&ø'Mu¿Û{–yS¨õ¿Üë±~è"R¿àþp·'©AGNbll3FGL J1151.4-1346PMN J1151-1347?ïþ–ι$?×#Œ½?&""µ×å?×#Œ½?ïóQ×k¿Ê?Z^"´Zr?Y\Q A[š?Z^"´Zr?ïø{¨Üœg?@3¦cÂM?N[ë`Ó)?@3¦cÂM?ïõ¢¯ö[?8Ô7dÆÇ?TzºõI™­?8Ô7dÆÇ?ïüôã?1Ï	^?8_~ëð_î?1Ï	^?ï϶Q"Ï?w#8a_?x$×6|	?w#8a_?ïö훊›¶?b3f‰tÑð?R$ÉUücL?b3f‰tÑð?ï؊¾	x?aÁ)°ônB?sº ü—œ;?aÁ)°ônBAGN4FGL J1151.5+5859?͘ä3¾@L>-b8Ú<À9¢àJXçÀ<U¡E@Ý\u éZ?ûY
Ð>?³ ôpTÒ?·9@þÍÐÙ@ÅÈFUNç@OKí"C?ä
¢»Jî¿ßBÌ-jœV¿ÕpàÝûÉ:¿Ý8 z´Q+¿ÙùÄ6%¿ã¸ãÁ…ñÇAGNbll3FGL J1151.4+5858TXS 1148+592?ïú"49?=•}ԅÑ?E¯.ÎP•^?=•}ԅÑ?ïìù›ž?`B¬P?c€ˆÝï?`B¬P?ïî!¯îZ?gÙw‹jí`?aÞPæsþ/?gÙw‹jí`?ïŸÛ9÷ól?e°B‰Ü?ˆ	1w´Q?e°B‰Ü?ïôÅYêô?Qêw?VuMFž6Å?Qêw?ï¼ð6ðhD?€á>"Ís"?€ÃòK?€á>"Ís"?﹑%`Q?†ƒ"؍?›»…Æ3Ç?†ƒ"؍?¿?ŒKæ)âsõ?¦µŽÒ@H?ŒKæ)âsõAGN4FGL J1151.6-2115¿Ý:Qàrq@CÀ¹w…r›À:üõÊò×ùÀ<–þï^È@ ~Þ¿¤ó?üáX"Ì?ÌëÔWÜ?»k/ùÂÏ?ñµ¡7Ì¿?ÿ8¤aHÅ¿ïênió9?ïò`ŠÚ9¿àh"¾é_U¿Ñ²ñCú€º¿ä
d½™Óü¿ØhÒý='íAGNbcuNVSS J115140-211345?ïþÅêOƒ?¹*?gÓ?#¯ï§Ÿ²w?¹*?gÓ?ïê6½Vb7?li¿Œe?eÉBžŸ¸?li¿Œe?ïåóíMî?xÕt±ØÎ?jäZq^?xÕt±ØÎ?ïÛÎÞRŽÌ?U[‡Œ
+m?rß§–?U[‡Œ
+m?ïþ¦xF°? $¦þúe]?&õ–ždۏ? $¦þúe]?ï£-ؑB?‰û.¶Ì°?‡4‰Ûœ¯Š?‰û.¶Ì°?ïÒ(\H2ý?ƒë`k®Þ?vëѹŠi•?ƒë`k®Þ?ïRul#ûÄ?'¹Ëd,»?•±RvYŠ?'¹Ëd,»AGN4FGL J1152.1+2837¿Ô%/%͸@S40@9«óÀ;aga8)<À<ć0
‰Ç@!?Žµâ¥?ýÀ(Ê#¥!?ʑ8wß`?W]άÖ?ÁåŠ2ôI@ù
¿cí¿íIn¾¤•÷?됫´NPÆ¿áѲ_c<æ¿áqùAŸÝ€¿¸½=ã^¿ß$ù9{øAGNbllGB6 J1152+2837?ïþ¸øã×?¯¡DÎå?$pnW
Èè?¯¡DÎå?ïö¾7ޓŸ?S~ ‹ÒŽß?Rƒ*'Ç?S~ ‹ÒŽß?ïñò+‰¤7?QÖÁ­àԑ?\¨Ã|BÑ?QÖÁ­àԑ?ïúø´‡0¶?1U8¥Hc?D-z<Jl?1U8¥Hc?ïþڄ£ò?&V†DP
?.BZ"Õ†ƒ?&V†DP
?ïÝץݎ€?t=MK‹çN?q-+UÇô?t=MK‹çN?ïî©»r(ß?k'à•"£?aVDÍðê?k'à•"£?ïç¿
±"¼?`x1€×9?h@õ"ìW?`x1€×9AGN4FGL J1152.3-0839¿ë'Ò`h(;@I¸ÿ!³®ïÀ91÷ÃœcÀ<¨Ü,¼@ïapˆSK@è#½tj?¯
^\N,?µIȔ.@|Úa
@å،s–?»kÂíC¿å;*®)s—¿åÁ »¿å󾩛¿ê"œý|B¿és$ºÊlAGNfsrq3FGL J1152.3-0841PKS B1149-084?ïü²7ö"?7,»DœJ?:n?Š«c?7,»DœJ?ïõIn;¥{?VÝùˆ«)v?Um#ÚC?VÝùˆ«)v?ïã¼ÿéôj?r§i+ûw?lCJE¥ÿ?r§i+ûw?ïýÈü™Õ:?!'tvؾ}?1¸mŸ¤ó?!'tvؾ}?ïüOþ‰Í
?2iÕõ45?=€3%ût?2iÕõ45?ïÏ«f ð?|8ÙÑþ?x*L±à?|8ÙÑþ?ïÓ2™§¨È?yxÃ<(šì?vf³"Œ³á?yxÃ<(šì?ïújÔ¬Œˆ?9X0;.Ƽ?FT­
/*?9X0;.ƼAGN4FGL J1152.8+3308¿ÈeÇQ…@RÿÀ6âëÀ:œÞÀXÀ<}׺f˜»@§õýȘ@´Å¿'Q§?¾]b wóñ¿½TÂá!Ô¢?þÍðÁ@Ÿ¶2+¡D¿Ô¦"Sß{%¿ìwÅü-ã¿ëÕ9¸ˆr*¿Ò¥ñ7"+¿é(ýOL?³E'Q}¡AGNfsrqB2 1150+33A?ïþ]-`>?,I4úä?.Ú(ð¾º?,I4úä?ïñ	ܼrÑ?bV¢½Éhƒ?]ìGÌLÅ?bV¢½Éhƒ?ïÈ7½¢?~h5UBÃÇ?{äx§fúÌ?~h5UBÃÇ?ï÷ó
þé?A½‹Öv‰?Pþˆ«??A½‹Öv‰?ïúÛyž+?GEBŠ?D'¸/"?GEBŠ?賓dßä¾?†œ¦÷øŠñ?…–æÎæ†?†œ¦÷øŠñ?ï¯c.g`P?…"]Á+?"'4]èÛý?…"]Á+?ï^Q€¿ò¹?Šm¨7Ëx?"5Ïä'ô?Šm¨7ËxAGN4FGL J1153.0+8056?ïèfuʖ@Aï îؐÀ:+jК¸À<_ÙSÃÌs@}à}Ù @Zt:dÜ?·hfEÚ*¿¯Œç.¢Õ­?ò×z:XÁb@ꗶ?—›?íº¾?©c¿äÌ°èj¸¿ê8±ø50¿æ¸/â縿ì̼¦äÛ·¿ïÿŸzFAGNfsrqS5 1150+81?ïüsML‰?=Çø¸•UÞ?<e•Ë»t?=Çø¸•UÞ?ïöëüuÃ?Uéš%l3x?R)gI‰c?Uéš%l3x?ïÚýë¹Þ?s¯H
¨¹?r
$pˎ?s¯H
¨¹?ïýǒ?$"''Ýnä?7¡ÂŠ»o?$"''Ýnä?ïûóîúŸ?CN²kbaI?@0D©6:?CN²kbaI?ïÙZ
ßÞð?r»M"¼{C?sRù?Ô?r»M"¼{C?ïؚ»­•¥?~¤%ŽPV?s²¢D²
c?~¤%ŽPV?ïóÆÿ-r)?I¨í+(¦I?Xr¥­Û?I¨í+(¦IAGN4FGL J1153.3-1104¿Ø8‹}³EM@H¤eƒèWmÀ9ð4îõÁÀ<6¶³…Óê@clùþ^?@0>Œ,Ê?·c´Û>˜?²ù¤)ëa?øopJ붝@8ßwŸHÛ¿Ålê¹ò«¿âõ}ðñš¿æt«"­ÿØ¿âvO¿êñxô¿Ù8ÊKéžAGNbcuPKS B1150-108?ïýø§#Îo? ò¨8¹,?0:ÆH·ƒ? ò¨8¹,?ïô ¢¸l?Zœ™uQѲ?V¾»íÏw\?Zœ™uQѲ?ïñw¿)K(?JéfÏ*"»?]{ïPb?JéfÏ*"»?ïÿ}Mªû
>ÿÊ^¬jõ?VGƒ@¯¢>ÿÊ^¬jõ?ïü¤EÅ/?1l‹ Zô…?:Ýд)?1l‹ Zô…?ïÐéE9¬/?~kÖ¸"ù¥?w‹]V´,?~kÖ¸"ù¥?ïèd'üœs?pC³ò×ìš?g›l¾«]"?pC³ò×ìš?ïþÜzè?ú¼¬Äè`?"84‰ë ?ú¼¬Äè`AGN4FGL J1153.4+4931?à0£«>î@P?W}•WÀ8Þê'ò#À<AÌN!Ì@˜ üö@ŽŠ#Û?¢Ã^äçˬ?£ãñ¬€&+?þäԕîê.@Hm²(‡¿Öыؾ¿äÔú˜¸¿å‹MpÌö¿ãs>í¿í=HËJ썿ß9Ü>YØAGNFSRQ3FGL J1153.4+49324C +49.22?ïýi×Móî?%£—h|?4±G=/Ñ?%£—h|?ï÷ìAˆ™?P#ÂØë¢?P'~;å?P#ÂØë¢?ïÖbŽÚ<¼?{[co'?tθ°nEü?{[co'?ïÿâÆ´.ñ>ë(âoÚ>í93%vŒ¬>ë(âoÚ?ïýsHՏr?*Oể¤?4e··µ?*Oể¤?ïà$쯧^?s"6ù^¶?oÛn•1?s"6ù^¶?ïåø—½?rͧË"?jáŒ&³V?rͧË"?ïÿå÷HÔä>ô&ÒtÈg¾>꧕3õ>ô&ÒtÈg¾AGN4FGL J1153.6-2553¿Üƒ+…%*@A–ÃÉîËûÀ:…wqP¥4À<mgZ',–@ BP¾ßNZ?ü5 *­R´?Ãõ]$H^¾?ÆÙHƘUL@1æaÉH´@Z9è4¿ïñ¸ðiŠ?ïE®*JVe?®@ê</—Y¿ß)¦W>
¿áÊ°]*}'¿ãž™]´'AGNbcu3FGL J1153.7-2555NVSS J115338-255412?ïÞôháڕ?­Ã/¬èl?p…Ëœ!9†?­Ã/¬èl?ïñB¢yg?]ñ•Ý	y?]{Ös•R%?]ñ•Ý	y?ïÚx
¶.?}Áά¡å=?rÃù^ç<?}Áά¡å=?ïçzÊÃÕz?MÞÏA‰û?h…5Ðî'?MÞÏA‰û?ïúcC¤Î	?Ejm"Ò€@?FròA‰Et?Ejm"Ò€@?ᅲ´ŒÜ?‰è;šJ?€?4¾å?‰è;šJ?ïÍtg_?€fta§i?yEøÖ¤=?€fta§i?ï´kƒj?nŒ'®hW0?'åI\m|?nŒ'®hW0AGN4FGL J1153.7+3822¿ï©Ô
•@R`{_ïJÀ;i°Œû%¦À<ç¥'lU"@ ¨RÑ^,?þ­é—Þ®w?É´—L?yœèƒŒ'ô?µm‰_(žI@vJ_É¿ï7óâ:rB¿ÊRŒ)nŽS¿Ð¢0aFÁÛ¿è'Ø¥H#…?Ã^jÄoF¿áPå*'¤AGNbllB3 1151+386?ïþ¡pB?áÉÝ,7?%èüšÉQ\?áÉÝ,7?ïø£¾T#?P©ôO£Ï?Mq—b>b?P©ôO£Ï?ïæšûæ¸(?lcۍØ	à?ieF¢¯ú?lcۍØ	à?ïþ	GýDº?ê® ½Ç?/kû²Ôy?ê® ½Ç?ïý=ϳì?0 Ô›Ø?6 rŒO?0 Ô›Ø?ïÞÝfße?uG˜"Ç!?p'L‰"•ƒ?uG˜"Ç!?ïâÊ–>"?s8ùáÏސ?m5ùha•S?s8ùáÏސ?ïö›•rB"?N7¢H¬õ?RÈÔËÃë+?N7¢H¬õAGN4FGL J1154.0-0010¿ìzìÅ»‹‡@M³þCg]ÝÀ:ÄÜ=ƒÀ<:贉ßè@ ¡Øñd?û¨À˜áãµ?¾(²?œ'à?®1´%Ÿ!?óêIš}Å(@ÉÌJØÁ?ï÷±j8X?¥^w.µ ¿ã?@óVµ¿ÔEO_¹£û¿ÉÁJ£g†¿æ-h¹&ý›AGNbll3FGL J1154.2-00101RXS J115404.9-001008?ïþAÞå\?+V³¾háO?+ïÂÕ`ϕ?+V³¾háO?ïò	Äh¾õ?cîGÆ(ú?[ìw™µåR?cîGÆ(ú?ïñŠ€ïK?jà¢,ë?\êý 8t?jà¢,ë?ïøIV{Ã?3ûé"Ûœ?NÚ¦·Ð,ì?3ûé"Ûœ?ïý[\5ú¨?-^¼Šÿd?5%¤ÔV?-^¼Šÿd?ïÏOC<É?x›\ŽÊ&?x~ØyÞ{<?x›\ŽÊ&?ïî®ç^žq?s'¿GœÞ?aQŽ#¿,?s'¿GœÞ?ïì9û<?S1ó¤É>Ë?cÆò†,n?S1ó¤É>ËAGN4FGL J1154.0+4037¿îžµ
y¡h@RؤTÞÀ:KO7u¸À<Kžd¶@ŽeÖÉzÞ@¡·D¥?»©¥Ö=ä½?žçÚø½7?âÙV}»Â@
€#½Ÿ]S?ï¹OýnUH¿¨³oX¨bµ¿áŒÈ›䟿á4Âkðê¿å:c©Ä\¿ÔdfÜØÞ~AGNfsrq3FGL J1153.4+4033B3 1151+408?ïþ'.(m™?§üþý°?- 'ÿe5?§üþý°?ï÷½e·?REzNñã?P…ÙÜra½?REzNñã?ï÷ƒJ³é?Dˆµz6a?PùjStµù?Dˆµz6a?ïóS–õ^?B¡
¹ã?YXÓúCn?B¡
¹ã?ïý)Ø°I£?+nPÕ<
?6±;p°ß?+nPÕ<
?ïáZý–]?pP½~Æo"?n¥p'%?pP½~Æo"?ïöq€¥?aŬ"Âs?SùdÌ&Ä?aŬ"Âs?ïä¨{HÈ?XJzð/¬,?kW…+²82?XJzð/¬,AGN4FGL J1154.0+6018¿î[" Íf6@K³û?¦ÞüÀ:Ý]=ȸÀ<FDw(UŠ@ý¤)j‡ˆ@j$aY?¸ÅxqÖ²?ÎÐd¾›‡@AÀ6@ÓÖ;‹qc?ÙêY¥Ã£¿âRƒÅò½ø¿é³ß¿ëÔ9~§¿ïþ{ ۑ?ïêӝ÷LRAGNfsrq3FGL J1154.3+6023RX J1154.0+6022?ïåŽB…X?kŽ˜R?jqòÒÿ'?kŽ˜R?ïót	£S?Y}cÿÁJ?Yí5ËF?Y}cÿÁJ?ïCËrôX?Ž0×Yãp?—†'£,Ê¡?Ž0×Yãp?ï꾫³æ?PñÿË?eATPq¿?PñÿË?ïÍÓ؄»ç?|Â0Là¸?yºâ\‰?|Â0Là¸?ïÈì"Ü¥?{I¤	­Ó?{‰îsð?{I¤	­Ó?íu&7¢-½?£[Oç•À?´VÎB€žš?£[Oç•À?ï܈pk<?KT—Oö?žnìË.?KT—OöAGN4FGL J1154.1-3243?ïeA°»@<Ÿ¡<%J<À9Tm'LžÀ;ñ´#ìn@"XWÚÝ\?þðCå2`?®wE0áŸB?¾ÁÀ	@t\!iT@
¨!"Šé?ð¿ÜÉ/^giq¿áª¿†¾ ¿ÙœF‡£Íпç¨S;wG¿í™šùdAGNbll3FGL J1154.0-3243PKS 1151-324?ïúõbãS?<{ð˜a§?D*v׏6?<{ð˜a§?ïà(°«â?zָͫ3?oô×W"-z?zָͫ3?ïÃ"Ù7®?œµC i?~n""uPÕ?œµC i?ïÈ0X7y"?]µSiP}?{çÔÅá?]µSiP}?ïñ–$'|6?luëy7+?\Ó·4ý"4?luëy7+?}/D€?›Ú'I?k? £Ô?›Ú'I?k?ïaA'Vtñ?"†OÙ¿Ëô?"×Û1aï?"†OÙ¿Ëô?ïÂ§Ò9?"¥î&X?-ç¢n²ï?"¥î&XAGN4FGL J1155.5-3418?â»>ÛïÔ@;%ðÃL‹À:=Áz‰3À<O»S'ÅA@ ³‹WŒƒÜ?ûъŸb0?¿ 8Åxr?³yx€´	K?öœÜ_@Ÿ1czN?ïþ»ýq°G¿ç$O€íl¿Ó¼GÃe¿Ð\¢õ¸Ô¿äbÐzw¿·Bï=åé©AGNbll3FGL J1155.4-3417NVSS J115520-341718?ïþÚÞÞGI?dÊhœë«?"Rç®xm?dÊhœë«?ïñÈÀVOv?`VCcñà?\na"Ê?`VCcñà?ïø{ÃW?RÄÒbÑò?Oîæ%À?RÄÒbÑò?ïñ*ތ# ?C*ÛÊt÷?]ªBÜ»Ã?C*ÛÊt÷?ïþÐ¥ŸaZ?Ù+•n?"õ¢%Â[?Ù+•n?ïËêS'ÆŽ?~"ô"¦â:?z
ÖP¹ÀÓ?~"ô"¦â:?ïù"3±»Ø?Z`"­(?I¯1¨ªV5?Z`"­(?ïÚ?ف2'?]¬¡ÅøFG?rà`böÚ?]¬¡ÅøFGAGN4FGL J1155.6-6547¿×8çÛ¤ŠÀR¶ä-;¢À9Ö%Ü2›^À;;u –
@Åv¼ƒ)@ê໗?ΛraÇEN?Õ« ,ZÒ@	WQ:…7?ôxƒ<
d?ïç)€=Ó¿áD7%?U¿é¤óÕORN¿ë¸ðvö£¿ïýwקò?˜cï=ºöŒAGNbcuWISEA J115414.97-654215.0?íí5¢p¥&?ÀO?8$3¼?°–RëžïÑ?ÀO?8$3¼?ß%>"?Яý¢òM?àm`¸sñ·?Яý¢òM?ì£BÁ+êü?¢d	\"ªJ?ºåéö ¨#?¢d	\"ªJ?áÅâÐ%-?³KUÉ0a?Üt;ú_µ¦?³KUÉ0a?éŽ57oWý?ÅﲤqRÂ?ÉÇ+"B ?ÅﲤqRÂ?·…6à(3?ÄНšbÊÙ?íY?È~?ÄНšbÊÙ?àï™f»?¹I`û…S?ßÀ!ÔÍ2‰?¹I`û…S?šÄUù¿p¯?Š
+Úwz?ï)ÝP‡›?Š
+ÚwzMIXED4FGL J1155.8+6137¿äbÂ0Là@K!ýÞ½À;˜Mà]£À=™0¾
í@!
øæ0K!?úèÎör¸"?жÙÛÓûÀ?ŵ¡bê"?ö¢XOLnn@)¬'½¨?í#·•-#O¿æÈóĈZ­¿æ×z:XÁb?»òð"wÍ¿ÝÉ/‰Z‡5¿ä,\\×qAGNbll3FGL J1155.9+6136SDSS J115548.40+613553.8?ïý',-Ÿ9?*ôwÈU¤î?6Ɲ³×Y?*ôwÈU¤î?ïóg¿	žB?X·X#´?Y0çD
?X·X#´?ïèӏDè#?jv>úªi?g,p…}õ¦?jv>úªi?ïç{
§Á?PCG+ƒ0g?h"õm‹æ×?PCG+ƒ0g?ïýdÅ°—?*K+Óogm?4ÙÑ5QO?*K+Óogm?ïÖ<Òï%½?tg>×Aø?tᖈm!l?tg>×Aø?ïæ"wŠaT?r=Š–C¾9?i݈™Zœ;?r=Š–C¾9?KÞû£?z>‡ºÓ?‰ÞmÑ{&?z>‡ºÓAGN4FGL J1156.6+0640¿âp;mOŸâ@PpmH÷QÀ;eEñ{ؾÀ<¾Lj;Ýý@HãHº.@q<î×í?Ø
PJ›.Å?Ó5ÂÅ+?õã]gº#}@
Ì3j¾9¿ïõð¢i÷À?ïö$´ë.¸¿Ñ·	ìèÌ¿å
ö~!)¿ïñÖ¤¿î×oZµAGNbcuTXS 1154+069?ï÷å?gýs?MÝlø›Ð?P5—a¦?MÝlø›Ð?ïõ%°Wù?Téí)íÃ?U´Ÿ…x?Téí)íÃ?ï#Ju1ª?<‰Î>t¬?›–±\ÙÊ·?<‰Î>t¬?ïï²hP)?G¾ók6a?`M—{œÚr?G¾ók6a?ïú-+?F®';Q°‡?GKT5èä?F®';Q°‡?ïÎxR:ú?{فW­·Æ?xÃÖÒÕ2?{فW­·Æ?îØOXdž+?˜-Û@¿?¢{
pY?˜-Û@¿?ïÐúäÀ½?h. £5f?wþ'«,EY?h. £5fAGN4FGL J1156.6-2248¿äˆàÜ@C+8`™ËÀ:mAaÊsÀ<_†z%@ð\ñržƒ?ÿ"òXwZ?ÜW¹û8ñ?ÄǏ¡F@"à¹(«@¹
¨4<¿ïÜl²°Â?ïÞÁÉ'¿Þ¢T~1‰:¿á[¹.׿ۢÉä:&¿èG犾4"AGNbll3FGL J1156.7-2250NVSS J115633-225004?ïûIï&,Ô?:´'•d˜?BØD*v~?:´'•d˜?ïæ´&㙘?g½ðB ?iKÙ*$Ø?g½ðB ?ïî)‰™ÏÓ?X¾Zh¶2¼?aÖvzÍÔô?X¾Zh¶2¼?ïÓbÄõW?Zb¥ô<C¥?vNþ)ãì‹?Zb¥ô<C¥?ïèÅíE0?aüHáÖTL?g:&h?aüHáÖTL?ïv²í[?"QªIä?‹û"Leq9?"QªIä?ïÌE@üÊ?ˆ£"Ï?yô]mïö¶?ˆ£"Ï?îþï§ÔV?Œ¨.PÙ? áÊì¡?Œ¨.PÙAGN4FGL J1158.5+4824?é蕼P@P—BÃÉîÌÀ:3(¦É-À<…bÎ+qž@iXûÓö@g6:N°g?¸bÓ3ïÕ? ®Ý½NÄM?âÆ8Éu)x@ O¼€ÏH?Ý	ß<fÏ¿äŠLŠN¿åµ‡k™¬¿çµ½A›"¿èWõ¹€¿Ýõy(àÉÚAGNfsrqGB1 1155+486?ïÿ
õ/^?ÚQÞ'{?A_ñ o'?ÚQÞ'{?ïø3ÂLJ¶?QFU6 >?O0óÛ£w?QFU6 >?ïõQsä¹?Sâ½åæ}?U]†tþÏ?Sâ½åæ}?ïÿÜ轈?ÐÔÈJ÷?Ä[TÅ$Ú?ÐÔÈJ÷?ïÿ<ã[/?·ÊcºÜ?|ž2±ºŒ?·ÊcºÜ?ïã[ȹÓÝ?p°Y6@›‰?l¤7†ÄÊ´?p°Y6@›‰?ïðËÏ?fìþ‰õð?_Êiݲà?fìþ‰õð?ïþJ#÷? hÚÚ¦øi?.Þ,3¹‡? hÚÚ¦øiAGN4FGL J1158.9+0818¿ïê=9á@PܵÜÆ?À;ˆCaÀ<§óv"Á›@ 6°Ë9yÉ?ý[ÛÈé~?Ê@åxjIö?¶ºùw]?î<G
ۊÖ?ÿj?›Ü??ï‰þ›üË¿íP_ÿD^¿ÃEyÇAGž¿ÚÚ¨!ò™¿ä‹ÂÁ[)œ¿Õl—£TYAGNbcu3FGL J1158.9+0818RX J1158.8+0819?ïþn?*m>R«?.!	­,@?*m>R«?ïì_–µÛç?f-Ì©Ø`?c iYBa?f-Ì©Ø`?ïõb|ÄC3?CºÃv'o?U;ó+‰°?CºÃv'o?ïÑ-½ÿ?ZË>¾¿á\?wi*²¤a?ZË>¾¿á\?ïþyz•Gz?!ÿÇÉ»?(hX=ô0ë?!ÿÇÉ»?ï®ÅGÈ@¡?Œ#'0øC¿?"N®Ïµ?Œ#'0øC¿?ïø©À¿^‹?\ßôTú¥ò?MXü5v½/?\ßôTú¥ò?ïQ;p]Nÿ?€Œ¤½0ñé?•Ø'ðæ"?€Œ¤½0ñéAGN4FGL J1159.0+0939?ӓ|DÛ7…@Q&8ÅCÀ9¼b †ˆEÀ<H}'ÒÕû@B™³šÌ @¥?|í'h?³Î#Žû[?°ý<aNÏ?ü«ÓXI@7}	Àóü¿àD'❪?ÓÚL|°TÇ¿ãU38;°°¿Þs]$žDú¿åÄz¿ç=W^‹¦'AGNbll3FGL J1158.8+0941GB6 J1158+0937?ïþàæ½Â?6«E'?'îdMl'?6«E'?ïõþC"¦?Z¶SN´«‡?Uü—÷D{?Z¶SN´«‡?ïóf{×^C?`î'Ÿ)?Y3àKW?`î'Ÿ)?ïùÁ]¿	&?3[:ï—?HúˆJ
"?3[:ï—?ïþ–¯j¢?"ÉX½WŒ?.'oí?"ÉX½WŒ?ïÓCJœJ=?|§"
»Ô?v^Z'ŽÃ?|§"
»Ô?ïïÒДNù?nrÅDmBN?`-/ž‹>`?nrÅDmBN?ïï´HÐ?PËU;aN%?`K·E÷e
?PËU;aN%AGN4FGL J1159.2-2227¿®Ì,p¤Âg@CjmŒ?À9/v>J¾jÀ;ÃQvëè@–Ÿ¤J¢'@Þ¥rðR?¶fŽ_0½?ÂKD÷Ö»¹@€	ö#l@3M™Þ?׀ÒbãÏô¿ã¶"v¿æ–îÄnYz¿åX³ UöW¿ênjЛ¿ïÿ~€8Ÿ"AGNbcu3FGL J1159.3-2226PKS 1156-221?ïù(í¬bÁ?JQ™î¨àÇ?K\Inä}{?JQ™î¨àÇ?ïô«À|v?[j_¬"\E?Wü¨"42?[j_¬"\E?ïÔj¦&¬?p#›ò•«?uÊ÷«ŒÒ?p#›ò•«?ïû[y‰"û?1)Ý'>?B'ò@þ?1)Ý'>?ïÛ¯é'*e?pAÃ>b¢?r(;ºA¸?pAÃ>b¢?ïÉV˜"	]?'ë–ԟ?{T³Ëù"?'ë–ԟ?î詾,¯?˜á'ÿT?¡ud!ê?˜á'ÿT?ïñ–"!žr?Nß"Â;?\Ò÷\Ž
"?Nß"Â;AGN4FGL J1159.3-2142¿Ñi©"¸@CÈú?̞ªÀ8ÞqÍ¢µ¢À;¡"ØaV@¸‹Í(<@çüÓû•?ªD?è<.?À·—FBÐ@á¼ýKð™@3®~Øù¿ÛTbWä¿âûîç´°¿å` ‰wãf¿ç9Â,_Ú¿éá1ޟ](¿ïþžÖð<>AGNfsrq3FGL J1159.2-2141PMN J1159-2142?ïöäKƒë?P£‡cËÿ5?R7Ïhø*ã?P£‡cËÿ5?ïè©¥!Ú?l£Õ§¥Â?güV›vÍ??l£Õ§¥Â?ïÒ´3è~ž?q¢Š3î«?v¥æ&¤î?q¢Š3î«?ïÜnDΈ†?VŸ­Þ‹ÃC?qÈݘÐõ?VŸ­Þ‹ÃC?ïë{ö4i?`Âm|Ê÷?d"
/¥•?`Âm|Ê÷?ï†ÿZ‹?¦säê€?!Ì|?¦säê€?ïÈ͎¾Ÿ?Ž¸@ëï?æV¿2
?Ž¸@ëï?îÚÖvD!?«žŠâJ!?¢RŸæãïì?«žŠâJ!AGN4FGL J1159.5+2914¿³ qÙú¶@S˜	¿œb¢À6Ù¾´Ü?À;tR¸3¹@
ÍËzgO@ӎ¢Å'F?‰ÕQðQ{?¯óæÖ¹5@"2~À¨@!æƒ.Äd¿Á8'Ù÷¿ß#½ßÉÿ"¿ã¤Û·K[H¿âóύd¿æT+
oÆ¿ç¶é¡éÜAGNfsrq3FGL J1159.5+2914Ton 599?ï÷Àðcz?KËW—[E?P~œ€Ý>?KËW—[E?ïè©@øåý?|¬ÿn¯?gV¿š£G?|¬ÿn¯?ïáÒ6)mô?wh¦9¹P?n-ÉúMü?wh¦9¹P?ïÿS…
EŽ?Rbh ã?Z>Ï»Ü?Rbh ã?ïõº	"@Ê?NBôY^?T‹íx¯ºP?NBôY^?ï¨:ê•=G?¬³ª¡Z¬j?…ñESÑvE?¬³ª¡Z¬j?ïçæÞhM?vàLÈ'?h!""e6?vàLÈ'?ïþTè Îþ?%?þhz?*±z}?%?þhzAGN4FGL J1159.5-0723¿³
m(†ã³@J¢qÿ÷œ"À:&Nɑ®êÀ<M@± ÷@¬úv~6'?üæ/Äé©|?ÆÉGÝc?ÅڿԖÆ@ÖÓßÅp@ò´/œû¤¿ïÿ틉5ž?ïüî×컿Þ7Ó@"TŽ¿ØoE2980¿ÚMâa®z¿íŒ_¿ƒ8.AGNbll3FGL J1159.6-0723PMN J1159-0723?ïýÜx!µî?&¥Œôƒ&?1=ˆ"Gç?&¥Œôƒ&?ïì¥ÏÕ7L?eöºÿãh?cZ/þÍ´T?eöºÿãh?ïâ8––Ò6?qèõTž?mÇiŽI'g?qèõTž?ïäî¬Eª?P¦0þ^8?kë…4µÒ?P¦0þ^8?ïûÍQ"+Ò?;+zâÅÔ:?@ʺTd˓?;+zâÅÔ:?ï¯FsÏ'?‹Ù«}RÙD?".bÿ­¯?‹Ù«}RÙD?ï·7l©?|ň?x¼d•ÿX?|ň?ï'Á•O÷©?xPßW[4?‹š¯q±Ä?xPßW[4AGN4FGL J1200.2+0201¿ÄDkeâó@O–#ûÀ:(*ùÀ<nΠâc7@Ý0õkL@Cx$Õ?½Æ'ÊBXë?½Àdß}©y@jä°a @\wûT¿âõõ»Ÿí¿Ý­† J¿á€>´pµu¿ÛYÄAê¿åSP¦^N¿æd¶}Õî´AGNbcu3FGL J1200.4+020287GB 115739.6+021927?ïþ¨'ü°P?M¢r6\D?%wÑP§ƒ‹?M¢r6\D?ïô«WÔt®?b'ŽPMêÖ?V©P([ó­?b'ŽPMêÖ?ïøs€ø…Z?TÎ֐8¨ƒ?N1û'â F?TÎ֐8¨ƒ?ïûd~ö?*ŠG'?Bnº"{?*ŠG'?ïþZJ?!q¼áNøê?*^'\YÐ?!q¼áNøê?ïÉï8mÀß?ŠÛÅ(·°æ?{cÖÞx?ŠÛÅ(·°æ?ï÷ØuÐ?]Ð#0ìé?PO À½­?]Ð#0ìé?ïñy¶¿-?Jùë8Ã
r?]'ø"5"?Jùë8Ã
rAGN4FGL J1200.6+1229¿êÆn( @QÉD=F²lÀ:^4Òo£ýÀ<v†oj@÷÷ÔãF·@"Í–&?Àíá\Ÿ?¼¥Ú5@)?ùý ª/@
|÷ÔÃ?í•÷ƒY¼4¿äy'"¿å79ó@ÔÜ¿åÒÑɋпå\ÏAS¿ïÿLa¢—AGNbll3FGL J1200.8+1228GB6 J1200+1230?ïþ4Øh¦ ?µ¢ƒ¡?,²uBKq?µ¢ƒ¡?ïóO'k¢?a›³¯*^¨?Y`ú²‰b¾?a›³¯*^¨?ïõ0+/ó?ZÂ•—Ó…?UŸáÛy?ZÂ•—Ó…?ïïý5uX?Fû¦&Ÿ?`ý¢¯0q?Fû¦&Ÿ?ïþ2ݚFà?"EvûP?,Ò(.J"?"EvûP?ïË^Ž¼×ó?~ԇI"'[?zP¸‡vþx?~ԇI"'[?ïñ2þìø?elè±eÛU?]š'Öv?elè±eÛU?ï¹úRŸ'¶?mŠÈ…gJù?kXË>ž?mŠÈ…gJùAGN4FGL J1200.7+2008¿ê¸ò%ÂÝ@Siì,äeÀ:´Ç‰¤À<l´ˆ2i	@Yï`÷'@âÿœ,ñÑ?·ƒÀë?©Ýì@Õæ?ð ó*.§³@	å·Îí?Ên¸ÅXå¿å­U¾xv3¿ç'ù¾ÈR?¿âÛ._ƒô¿ïþ|§ñK1?ïÚ¡–'õAGNbcu3FGL J1200.9+2010TXS 1158+204?ïûÀ­rŒ?7P°ŠMñö?@ÿ˜`aØ?7P°ŠMñö?ïõEVBÏ*?W'‹¸!pp?UuStâL0?W'‹¸!pp?ïÍ[T(e?€.ÝqÞà?yRUàʯ?€.ÝqÞà?ïõÌìå?D¢_'Þ¦?Tgߣñ6¼?D¢_'Þ¦?ïùóº*}?FGÉ%B8é?H1L2Þ?FGÉ%B8é?ïÑÿP?}dX'j®k?wW츓ò?}dX'j®k?ïÞÑmpú?z7ӊé'?p—=˜Öí?z7ӊé'?ïȘ\z Ð?oG)teQ?{³Ñ½p8?oG)teQAGN4FGL J1200.8-1429¿ã —±{ÒM@GMØ@žUÁÀ:é'm{.À<vRNmS@ VÀ"Ûë?þöíï/Î?Ë«¾à%??¸·²3nlo?ìç¬sßÌ@CIËûìu?Àw¿ïçågÎE?îYœô—ìñ¿äˆ-@U¿¿×vÝâžÆ)¿à¹Ö?è"iAGNbcu3FGL J1200.9-1432NVSS J120055-143040?ïþà±8Ð4?ÿÏ.*Ý!?!ôëUE»?ÿÏ.*Ý!?ïô½Ê%}"?Wx)ý•o¦?V"kLº•?Wx)ý•o¦?ïöŽ]Þ?VT'tu.?SÀãlAãÍ?VT'tu.?ïö%Ó%
?@_+'œ'?S´Y½y[U?@_+'œ'?ïÿÉ8B½?y™öíüØ?†Ô#΍ê?y™öíüØ?ï˧*ѺÈ?€oEN	?z,j¯/ßÀ?€oEN	?ïö»JeÌ/?hîà·R«?R‰kyт?hîà·R«?ïè7e-<Š?`
‡¶ÅßÖ?gȚÑc§?`
‡¶ÅßÖAGN4FGL J1201.1-0332¿ïwO'þ@L'"¦óõÀ;Ô/—@À<nê™fn@Hÿ¥è?þ­[î=_Ý?̇'™£?ÆÂáfŒÑà?ý¯3^Ò@ Ü2ÆQ¿ïÿÀà/€ ?î.-À,«Z?ìNÛ?JB¿Þ…pí¨åg¿çvFŸ¿à)¥÷ÞÉAGNbcuNVSS J120111-033219?ïý2Áâþ?,ãfØdzH?7~kÇ\ì?,ãfØdzH?ïÖvµ¥$#?wBKú^fL?tÄ¥4M&´?wBKú^fL?ïáÎmƒ3?m¯‹¤?nú1T£Õº?m¯‹¤?ïotH7?z˜aÃæày?'1vùR?z˜aÃæày?ï÷AÀi½?I¾'k±}1?Q|~®Pž?I¾'k±}1?ï{Ÿ'x?' b+¦ô?œ,€™z?' b+¦ô?ïœõI¡<Y?‡jOþ:Æ	?ˆÂ­ž!Á?‡jOþ:Æ	?îFáΑø?›^µºXù8?«'ãÂ…?›^µºXù8AGN4FGL J1201.7+1429?í°š¿´`o@R7UqKœ·À:'£.mѕÀ<'ÌK@!'Mš¾@oªÛ
}2?Ó?ÅíhN?םÊD\P?ýS'i#°@×Ç7a–¿Öùœ#6»Ô¿Üéwލ¿àѦPaAc¿êC¡É¿ïÿüÚ±'Þ?ïÿá∠ÎAGNbllOM 198?ï癴>?dͯûw±p?hfKå¹ß1?dͯûw±p?ïð×À4§Á?aƒiá­õë?^PI¹=î?aƒiá­õë?î@UýQhÂ?›cœ5Ï?«ú )1¥à?›cœ5Ï?ïÜ-ß–Ë?_çԒÏ]?qéRÈÉ?_çԒÏ]?ïÅðBÙՅ?'!'ŸýZ?}ވÆi…?'!'ŸýZ?ïžQéùû¦?·¢šÔj?ˆk…w2Bq?·¢šÔj?ìôâÇyÀz?¤F´˜hT?¸XéÂè!±?¤F´˜hT?ïS»œ^?ŽZâ{j?œUˆßp8?ŽZâ{jAGN4FGL J1202.4+4442¿ÔI"*>{@Qw#x«‰À;7˜ólÀ<´"!Š"C@§§·§þ@xd"?Á]m
¦‡¿µsd%Ä`?ô
®ñð@/!Û¬º¿ÚícV˜¿ê"›Oe™¿ßŶƒ	_O¿çCO¢Ý¿ã¹Ë¾.ú>¿ïÿÿ)@k*AGNbllB3 1159+450?ïüO9´~?46
àõ?=†2%ª
É?46
àõ?ïîÏëÆ?_™ÜyÙJ?a0ê\
²?_™ÜyÙJ?ïÊâהì?zÄ×|Õpç?zýŽŸ4J?zÄ×|Õpç?ï欞Òé?RÓã–a±™?iSéA®º?RÓã–a±™?ïû"szÿƒ?F7¶ýkі?Cv2»®â??F7¶ýkі?ï«Ä{¼Ü6?‡mP—Ew?…á!öþW?‡mP—Ew?﯅ֻ…t?ƒ{öÜ?"ŠFÏÏ	?ƒ{öÜ?îÙ:^J¹?"¦"+í®?¢lZÀºG?"¦"+í®AGN4FGL J1202.5-0528?uÄyA4@K©›ý÷èÀ:+L''ÙÀ<;µ%ç@[§c0ÑÚ@OãÖԎ?Á¸v¾ù$š?Áâôq¯›?öcLŠÅÁ@ztJ»?ïÿýaw¿çßlâj¿ê˜"t¼j¿êzª@/ðÞ¿ïÿv}_Ò#?ïücÈý4tAGNfsrqPKS 1200-051?ï±G«eI?´zY(äpp?ƒ®7€Õ?´zY(äpp?ïô/Ñ|_?X˃(?W¡ÁñÓr¨?X˃(?1J-~?Š۬ō—?‰Ý³¾¢¬W?Š۬ō—?ïÿÅVXI?Ïr–¥Ä?gZ{º?Ïr–¥Ä?ïù"=EA?PÃGL?I³L×
ý?PÃGL?ïҞ>Þ¦Ù?z´«ÒÛ÷d?v°àü§¦?z´«ÒÛ÷d?ïNçsŽr?'êY'§é½?–#–Å»?'êY'§é½?ïû5
©&?9D&̊PÆ?C+«ç¼û?9D&̊PÆAGN4FGL J1202.5+3852¿ê¢j÷ÖÌç@Rœ;÷'jÀ:h/"BAÄÀ<'{ZqÍ@d[ô@ÈÒDŽ?µg×)È¿¬×ä>Œ
?õD5¹ö0@¡$29c#?ïÿíáoq'¿â£Éh">¿êsҕc©ô¿àyÈþáòÏ¿ã=š)âQ™¿Áù CVíAGNbll3FGL J1203.2+3847NVSS J120257+385147?ïûó´ÿ6é?R™Â‹?@1,›ùc|?R™Â‹?ïôï¼Í?T‡Ä%ҁ&?V †eèů?T‡Ä%ҁ&?ïå½pR<?pgK<a(¾?jêB»¨Ãq?pgK<a(¾?ïä!wÉæ?Qj܂ zû?kވ`µ,?Qj܂ zû?ïô~wTJZ?VP©?óî?Wp({±?VP©?óî?ïÍÀe
pÇ?zŽ.ÂXô?yÍbºXƒ?zŽ.ÂXô?ïÈ·A¨Êm?€ÔT¥ðÔ?{¤_M5É?€ÔT¥ðÔ?ï8íã®÷¶?††¹¬¯W
?˜âC'A9?††¹¬¯W
AGN4FGL J1202.9+5141¿ÑvBwî¨@Oå¡ÊÀƒÀ;CZPÀ<¢¬k-u"@O€íl@'¶'!%?Á"íå÷K¿´í¤ˆµñ"?õÕÛiGÂ@]Öÿž?ïܲø¿êbÑñÏ»•¿ç¿:¨rzq¿á×¼_AY¿æ¶ÇÝyÃ:¿±?štµßuAGNbcuTXS 1200+519?ïüɂü…]?*ÐÑì¡?9³æ•w0?*ÐÑì¡?ïë?YV†?fN³jCÌN?dÀ¦âL!×?fN³jCÌN?ïèÖ^,A?d ì7õY?gô)å,@?d ì7õY?ïß^Ԑ?ZNÓOƒX?puðµ×æ?ZNÓOƒX?ïû†ì÷BJ?>9
(F?AäL"rV?>9
(F? ´·?Oœ—È*ž?ŽÿBnN?Oœ—È*ž?ïÒVQÎÝQ?z¼–
þ=?vÔ×#ƒ?z¼–
þ=?înrŠÈ<?™í" Éöš?©×\/Ç<?™í" ÉöšAGN4FGL J1203.1+6031?µÈ¿ZRÅ@Kη#îÒÀ9zû¾QßÇÀ<o*þ±K@vò	óï@n—Oß;?¬èÿ¡?³`ËqØàV@^—eóS@	'R á·k?ï7Ÿçòm¿àBD]§ûÝ¿à'Y«m´¿á*i*f¿éV[¡'_¹¿Ð¥ÁۂOAGNbll3FGL J1203.1+6029SBS 1200+608?ïüuâ¸Ïó?2ºšß?<P镬Ÿù?2ºšß?ïï1ÅÛþ?k!ß$ ?`äÎÉ*A?k!ß$ ?ïâ–ÃPw<?q÷©u&ï?mi<ÞCsó?q÷©u&ï?ï{ëMkn?y˜òwv7?œBžé˜=?y˜òwv7?ïõx«7|?Qá Ï'û?UûãJx+?Qá Ï'û?ïÕ)7[áÓ?sÃÜ<o/­?ukdR¿r?sÃÜ<o/­?ï|¥FdØ?2§M­?kW1­0¬?2§M­?îc"<;?–i	ü$ –?©Ïî:;ØL?–i	ü$ –AGN4FGL J1203.3+1119?Ú5å%oas@Q¤_ !¸À:ç²7PþÀ<oIÊFá@7½%•ç@9'åøí½?͎8½`É?ÑޚTª|@iåvç¾@Ú¼ñ?ì[²BÝË"¿â¿ˆ¬Œ%¿çŽx¾­¥?¿×ž·æ‹º´¿ïÿù_|è3¿Áœª2AGNbcuTXS 1200+115?ïôôž¢íÖ?P€äGŽô?VÂ;²´L?P€äGŽô?ïì@2J*?b™–ˆ ƒ?c¿Íè°	?b™–ˆ ƒ?ï«pHèQ8?ƒ Ï¾ý«?…#íÂ|?ƒ Ï¾ý«?ïÓÜۅÐ?[~rLÔ¿?v'RÁ+¤?[~rLÔ¿?ïöfU8Z~?T¥ÛÄ{ã?S3Uôÿrô?T¥ÛÄ{ã?ý#_^?"«oý5lÁ?‰ß€©i¸"?"«oý5lÁ?ï|3ƒK_¶?>¾¶ò`~?y´ÑI?>¾¶ò`~?îՐ5ã?‹2R‹á?¢¦ü¬ÚL?‹2R‹áAGN4FGL J1203.4-3925¿çÒS"/@6'‹â÷±}À:?Ï)è1À<INiŸ
@!*øé‹I?üב#'?·IӞ"?p?yùø²ŒbW?Åù çÁÆ@BÝJHy?éj‹#µî?䯂~õÔX¿ÞÀù"æ¯!¿á£œ*Øò¿ÒÜÍ Öy¿Ðå×?—ožAGNbll3FGL J1203.5-3925PMN J1203-3926?ïûÇG²?2¥4¾¬þ?@ãïi~$?2¥4¾¬þ?ïﶰ'Á?`œ~ˆ£?`IîIíßj?`œ~ˆ£?ïîaĸx¤?b 7ÄŞ?až;
Íì?b 7ÄŞ?ïï$Xó?K[Çõ'?`ÛíŽOÄÒ?K[Çõ'?ïõÌ4÷X'?Nà®FŒ^;?Tg•¼S?Nà®FŒ^;?ïÊ;á¾²"?›î3Sm?zâ!V¢?›î3Sm?ï䕱¶#œ?v€»®ÉU?kjNhô=?v€»®ÉU?ïÔ{¢´?fï(á-~?uÂ.œID?fï(á-~AGN4FGL J1204.0+1146?åUÔÖ0£·@QÂûÒsÕ»À:w<
rIÉÀ<a
ž¿s@ ž^/‹2ù?üƒŠ´#ˆ›?ÄE´£ú?ÀRb"‰î?þy*X™J@
¢î$î¿ïÿýaw?ïÿþBe«+¿á1õ°ñ¤ó¿Ö¸_˜1¿Ù×i]ç'Ê¿ê0S'ˆAGNbll3FGL J1204.0+11441RXS J120413.0+114549?ïý¥o±"?,ƒ9ˆÒÕ?2ԁ½&?,ƒ9ˆÒÕ?ïìCǪú?c>g;ôÝî?cÿ¼;¶?c>g;ôÝî?ïÕ['T>?}ӇÌɏ?uRlWðÃ~?}ӇÌɏ?ïُáßÙ?Yª†Í¡Js?s}8oëG?Yª†Í¡Js?ïø¦wx‡{?Gµ‰ý€Üý?Mf"­ëL?Gµ‰ý€Üý?ï¦Â;ú,,?"ž:Úé?†OqÃÉ?"ž:Úé?ï'·Uí?…›xrÖ¬ã?z¡¤hGA©?…›xrÖ¬ã?ïHåî˔?…ý®a¿È?–ãB&Ò?…ý®a¿ÈAGN4FGL J1204.2-0709?ïÝÌ2n†@Jî`RP/À9nsbÎ+À;ÿ;"G@çß†Î?ü«åÌx7?µ#	ðCÊZ?µ—ÈAíá@.º'®›@—`,'?ïú·‹òçê¿äa©0'¿ßÝB»¼Y¿ÑÀ· jÄ¿âå4!Å¢Œ¿Þ•P^½$¹AGNbll3FGL J1204.3-07081RXS J120417.0-070959?ïþÀ–ÍPD?{	:+??#ö'nÇÙd?{	:+??ïðüûFes?bӜ­qÔ?^	puj²?bӜ­qÔ?ïöÚÏ«
?Hºr"3ku?SàJq(j?Hºr"3ku?ïë,ïLS–?MîÅàUÎ?dÓ¶lS?MîÅàUÎ?ïþZ{¢? 
RòՃ?*XK'šâÈ? 
RòՃ?ï¼Ö²K8°?•šBŠ3ã?€ÊSx0"ö?•šBŠ3ã?ïäé²íÜ?w<öMH6?kìon;·?w<öMH6?ïÊ1g‰¯Ÿ?fÓGƁD?zçLYdÀ2?fÓGƁDAGN4FGL J1204.8+0407?Èú;J@P7!Õ<ÞÀ;?ÐÐgŒÀ<~ÐV©Z@xB÷¡aº@ØÄ$"õ?Ðú? Ò2'?»æ;èך?èýpÇZ@	}=*WíR?惠žp˜ï¿êÉüÙ´¿â~wiÃèø¿ç5Š€Ìï¿ïöþdŠ¿ïÿñQçSaAGNfsrq3FGL J1205.4+0412MG1 J120448+0408?ïýÄ7ƒ`?+õûT-S?1ßÜYƒ'£?+õûT-S?ïôìÌ¡ò?Võ[—Aƒæ?V&g†ÃœV?Võ[—Aƒæ?ïÌ £èÁº?uÌq®Q5J?y¯­ÿ@‹5?uÌq®Q5J?ïõaõy¥o?>c$Bwš?U<vË?>c$Bwš?ïÿ$A#j?åZ³Ó"?wäG¯u8?åZ³Ó"?ïÆԁ2UÏ?Š÷ª3)T?|•¿‰10h?Š÷ª3)T?ïÙmíÌÕ9?~kŠÒÖK?sI	)c—z?~kŠÒÖK?ïπ|£Oâ?dsUûÈ­j?x?ÁŽ»/?dsUûÈ­jAGN4FGL J1205.7-2635?ÇmW"²@A"÷ µíÀ9mc¨FÇÀ<$
­,*@@SÃ÷f(@¥­Ûp?¯—d53¾?£9F? ô?ñ*MFðP@
cÒÃù"?ãR+Sk¿äå^ÿiؿ跍¹ç¿äNüm¾I¿èñžBuÆ¿â¸Æ báwAGNfsrq3FGL J1205.8-2636PKS 1203-26?ïý0w
Ÿó?&³\šÍ#í?6|H©-'h?&³\šÍ#í?ïô`X™?X~E"Ò—&?W?Á£=ì?X~E"Ò—&?ïë‡Ò4&?bʾÀ+ë?dxâr"	˜?bʾÀ+ë?ïøº<‹*?<™VG¦	Ú?M
§
Z?<™VG¦	Ú?ïúÂY^ô‹?:ð<"?Dö›l¹ÊR?:ð<"?ïËýo¨?;+ÖAÈ|?zH˜âÇÛ?;+ÖAÈ|?ïÝkn¹á?v¾Y]d˜/?qJ@Gó#™?v¾Y]d˜/?ïæÈ«¢R?]
rµ1?i7T€	û?]
rµ1AGN4FGL J1205.8+3321¿Õ¾7©öš7@S—àÞ҉À:êj€§ZLÀ<'Æp'9S@réîñÐ@
þ`Ï6?Åhî
¿†ý±Wa¡í?À"‰õŒ´"@òý
':¿Ö® ¤»5Ì¿é9ˆ·Ê¿å½Ëb>Ž†¿ãe"bøô¿î	܍40‰¿ï½ A"ôAGNbcu3FGL J1205.9+3315SDSS J120542.82+332146.9?ïý¦üP?(	'aŠ–N?2È­‰Œ'?(	'aŠ–N?ï÷TÜ@?NóLmØ?QVýU"PÁ?NóLmØ?ïêÓQ1‡?h#÷´û,?e,®Ú×{?h#÷´û,?ï÷™÷Yà"?:w­³)È?PÌA@$?:w­³)È?ïýÔdÜ¥?+í«u'?1\ÝFkR¨?+í«u'?ïÞ¯Ü.È?qG‰¦OÙ?p¨Íš?qG‰¦OÙ?ïòÇáŽ?aû^ý.Èú?ZqÝû¹Ã\?aû^ý.Èú?ïÔ5Öjt,?f'AÆ…N?uå´~-?f'AÆ…NAGN4FGL J1207.2-0524?í¨sÃ@Kàw¯dÀ;ÜÂä¿À<œ¤ÁëÈ;@ ™o¬5R?ù-Æèk?֒ÐÝR«ô?Ý
³ö«˜@x÷…@±ü/æÍ¿ìNá¿Î¼?ï{ìàh‹¿Ñöã•Ò¿Ó>úç'Jñ¿ß='üft¿ðAGNbcu1RXS J120722.5-052442?ïùS%kõG?M;ì¬È‡?J³i¤¤Í?M;ì¬È‡?ïâ'螲?j
—™?|?mrØ+þö?j
—™?|?ï®'qDL?{Oã0Q,Ÿ?"v#½[U?{Oã0Q,Ÿ?ïÈ7é?8?bK嵿¨—?{änÒRi?bK嵿¨—?ïù­^%,é?HPÍ¿
?IJ‡(Ç h?HPÍ¿
?>qæÞ?ŒføKoƒà?‡[0UÇØ}?ŒføKoƒà?ï­¼­´p?…cž'K]?"Ô–H@?…cž'K]?ï3ñ_/?‡¹SÃj†?™žaØÌ°(?‡¹SÃj†AGN4FGL J1207.7-0106¿ÚÐnˆÚë°@Mï÷øʂÀ:"ºˆýj$À<e*F$§@Î]Àz"@ÇúBPÝh?Àø==ù
?ÆÚ9ÝFl¡@ŒXž&Ç@éÉl|«?ïïZ@hOö¿ÑiدY¿ç&Zݜ'é¿á"?B
;˜¿é>ê¡tˆ¿ðAGNfsrqAT20G J120741-010630?ïÊK,›‹Ú?®_XÓqOÐ?zÚi³™ë9?®_XÓqOÐ?ïô†œõ€?Yî'ÐòÖ2?VóʽÕðV?Yî'ÐòÖ2?ïºÉeº?|
Xnº?zÍ­»±?|
Xnº?ïý»j']p?&ÜHµ?2$«
áˆ?&ÜHµ?ïë-íÆcô?`c$Ԑ?dÒ:ûã–?`c$Ԑ?ïƎÓªÉ?'ߥʰäù?|¸–zyo?'ߥʰäù?îÖ«œÀ.s?˜ïbƒ?Ö~?¢•F2EJÙ?˜ïbƒ?Ö~?ïúܯîś?65$¡!Í?D@RG$?65$¡!ÍAGN4FGL J1207.7-2229?åH&IaÉ@C£vfœíÀ:[§ºÄŒŒÀ<e¬9¯@DÛ½€?ÿ¾›ÌyÀ¶?Á7°év?±ô¬¶¬Ð?ñãUŠv(@Š`Á‹Ñ?ïÇ~¿M³<¿âg1g™¿ãåóö¿Ûp°½"Û¿ÞÆwž5@¿æèþ[»AGNbll3FGL J1207.6-2232NVSS J120736-223036?ïþƒççÁ?˜WÝâÓ?'Á"LjëÑ?˜WÝâÓ?ïôãõ2q—?YfКêØù?V8Ün?YfКêØù?ïúCÊUŠ?SaØ:¨Ã9?FóéOY?SaØ:¨Ã9?ïøGñ ²?2Ǘ³_ ?Nà9 Ѥ?2Ǘ³_ ?ïþ{)Í?ن¤mj?(O;eÃÙð?ن¤mj?ïėze?Ž^£ÞÈÌ?}´}¹Qåb?Ž^£ÞÈÌ?ïü¥lƒv?AvüFgY­?:ԛ؇«k?AvüFgY­?ïè%w]Ú?R×1ÿ#Z§?gpڛßõj?R×1ÿ#Z§AGN4FGL J1208.1+3017¿î9ᇆ@Sÿf¥P‡À;x+¾Ê«ŠÀ<Пe‹u@!KQŽ½ók?øœ bv?Ô\™`?ПäâBTä?ùÕ¢y<,@\<ŽÑ"ˆ¿ëÀnºÈ¾J¿ïûmÊö?ÒÊM8ßð¿Òk.óŠ§¿áì^Á¿Ô1»¬éØAGNbllGB6 J1208+3015?ïéÄDƌ? d2s^‹?f;º÷{aÌ? d2s^‹?ïô¡¯Š6?[-Ö)ÓE/?V¼ æZ3?[-Ö)ÓE/?ïÜíwðu?w•åÊ¿•M?q‰Dw'M¨?w•åÊ¿•M?ïì㼎¢V?NÞö¡Në?cC…ûQü?NÞö¡Në?ïý;áÇIš?=RÆ·b?6 ðeÛ2Š?=RÆ·b?ïÙOóÄn–?vÆ&Æ{ï?sX1¶q?vÆ&Æ{ï?ïë)Ü»Ç?p%RaW!?dÖqûhÁ3?p%RaW!?ïÁÐâÜË?pÿ£ö!Ã?Ž¥ìVŠ?pÿ£ö!ÃAGN4FGL J1208.2-7810?âÃ8DÑ&ŠÀ/d"À:¬#Ï!kÀ<hýwƒ–@ =÷¼d ?ÿjj6Õ#?ʳiäËG?³Ÿ€ŽZÌ)?éõv¤¢X?óŠy?­¿å2 -"¿çâ/jPÖ²¿Û¯~ˆF5¿Ûo/BÄ#¿á@¤Ö
¾/¿å!	ۂrAGNbcu3FGL J1208.2-7810cPKS 1205-778?ïûZy¦¾?b•ê˜{À¢?Aʕõ\Ý?b•ê˜{À¢?ïÛÀ³8ü÷?|øq­¶ï?r¦GT¸Ì?|øq­¶ï?ïåì)Îu?p6wcv`q?jÖ%'òÁ?p6wcv`q?ïÇ÷Y#˜ó?aM0ŸW;?|SZõ¶Ò?aM0ŸW;?ïúè`üð?Gi‡0}Â?D^{Ëí¶	?Gi‡0}Â?ï@òO­C?¨Ò¨8UÍ`?—á¶
_÷¯?¨Ò¨8UÍ`?ï厣'ŒÉ?tžQ"F?jq\z³‡"?tžQ"F?îm#¹ûƒ?—e93¶'?©-Ädl'Û?—e93¶'AGN4FGL J1208.4+6121?ï÷whä'@K'BZîc À;Gy;UAÀ<ãÚ\ØH@þèL/-•@ü÷¢cl·?Á±Ýˆ0æ}¿£ýÛb'Ő?á¨áJÞ @	·ïEÀ¿íÜ3rSοÚ\uâ/_"¿æoÚ•[œ¿â,ûv-ƒÇ¿¨`Ž­K ¿ë

"ZAGNbllRGB J1208+613?ïÿP\Á?	+÷³(m5?ýÏ­…G¼?	+÷³(m5?ï÷éD–v¾?R0(³p¹à?P-w1ŸÒ?R0(³p¹à?ï÷폐	?Uôyˆ?P$á"7šs?Uôyˆ?ïÿ)ëXK?
ì£x?Ú¼°oÓ?
ì£x?ïþ»P'Xv?$…(í=œ'?$JòÊUD3?$…(í=œ'?ïá»DËGM?r
aÚl?nDºü_w?r
aÚl?ïø¾Ïwæ°?YDö‡w?MÁÏIp?YDö‡w?ïûAí`@2?9LK° Ë?BøIçC­Œ?9LK° ËAGN4FGL J1208.8-1751?ïNŠv³]@EêÖ¡aä÷À:ë‡ß\òIÀ<~ϙ/çN@x¤ÉM'X?úøihyf?ئးø?ߚOa'C@I	¼AdN@JdJ,sü?ëÈì}—/‡¿ìWàðñ¿ÑƒÞÐZv¿ÜgŸKŠB¿î]UE¬²¿ïÿ韖]ÐAGNbcuNVSS J120856-175647?ïÏð›^Þ?q=²Ó¨d]?x²X"´Ü?q=²Ó¨d]?^_Y?‰ûé‡ýì©?‰Ý(ˆ¶ý–?‰ûé‡ýì©?î	Àj‹1?'£%䊌?¦/cûô?'£%䊌?îĀÛæ"è?ƒÂP˜,ã?£·ò?æ†?ƒÂP˜,ã?ïp`-ùH½?ŠðtõÎÍ?'óú;¯~i?ŠðtõÎÍ?î¥Is˜Ô?¬§aM4ל?¥«hÎör¹?¬§aM4ל?í9`^íÿ«?¤ð<¨!Ó­?¶4ý	ÙÝ&?¤ð<¨!Ó­?ë¯}¦ÉØÒ?¥Ÿëµs©k?ÁB	d؜º?¥Ÿëµs©kAGN4FGL J1208.8-2754¿êšÿoXÊ¿@AԀuÀ:œ(MüãÀ<añvÐ@ö@ˆÂ‡y†?ü~†ƒ<`?ÔS—VÉ:q?Ó#ç{NÕÑ@Ù櫛#Ý@é?'³"W¿ïÿŸ½ 	?ïî'ð2,£¿ã°E!óé¿Â½§€b¿èÎÁŒ&ê¿ïÿüoQÇsAGNbcuNVSS J120900-275350?ïë!œ»j­?px÷yOøh?dÞct¯Úm?px÷yOøh?ïäc˜fúÇ?lÆ)ÒtF?kœg¤øÚ?lÆ)ÒtF?g¬?‰*a؁Á?' Jä"î?‰*a؁Á?ﻼpÖy@?bíì¶Xã?ãØ Ø?bíì¶Xã?ï°­B "~?‰E}N ?ƒÔ¯m4£?‰E}N ?ï©ôÛ8¬?…[!É/\°?…'ÉFÑÝ?…[!É/\°?î]?Šâû? 2ZkŽ ?ª.¬¾R? 2ZkŽ ?îÞ¿zB«?lÛry¸?¢W‰Ì?lÛry¸AGN4FGL J1208.9+5441¿è'€4»@N­gý?[`À8¼iuå_kÀ<Bá³
Þæ@Œì‡¨*@é»ðÜw?¡$åhd1?²·z«ð@`"~@'¤¦½ïd¿Õï5­`÷¿äþ'"o¿çñ¢4rοæñùý‡¼¿î™pI>7s¿ïń~ªTþAGNfsrq3FGL J1208.7+5442TXS 1206+549?ïû©j"k?:Àªn[GQ?CýZpºö?:Àªn[GQ?ïö0-šB?UõY‹õ¼?SŸ¤Ÿ€ê?UõY‹õ¼?ﷇGK\ä?~3ãÿ»Ç?'.0ðXÝ?~3ãÿ»Ç?ïüP¼
Àf?1E'×–?=z`'s¦?1E'×–?ïü¶ÛRÍ?1¡šPE?:O"Æ  ?1¡šPE?ïÞ õÕ?qUÁŒ¬"?pø÷bv'ˆ?qUÁŒ¬"?ïÀÉOR4?"	/«Ä]?›q¹jj8?"	/«Ä]?ï÷ÈJBU?GuW' àà?QÖoÄg0?GuW' ààAGN4FGL J1209.0-4630?ïìS@ÕïG@/~ÀÖõD»À;"G¡A)À<`émƒÐ@0\"*š@mgâghÅ?ÍçΰқC?£ÝT Á?ٟ"ÛCÝû?þ›©¡¤ý?è,ck	cV?ÍYþí[c¿ë7»ûS¿Ðzý©8ž¿â£Ÿ¬Ù¿ïá½?6.AGNbcuSUMSS J120905-462944?ïûLÿÕÁ?Læá3½Rˆ?BÏÃ>èÄ?Læá3½Rˆ?ïÓǒÑ(|?^¥têÎ?v6·)Ä?^¥têÎ?ïÜ®ùõqS?i:gÌlQ?q¨ƒôÂP?i:gÌlQ?ïìWôøT?GöÛ·ð¬?cé§àl"h?GöÛ·ð¬?ïç¬_w'f?j4-
ê?hS o°iÐ?j4-
ê?ï0o(׺'?¥œì¼)²?™òê0Ç?¥œì¼)²?]Mõ?‰·Ãé2åÚ?ˆ×(ºA+…?‰·Ãé2åÚ?ïyÔå'
?›û+Ùol?Åc^匹?›û+ÙolAGN4FGL J1209.4+4118?ç'‹	^@RY•ÔèûÀ9¯¡BÛGÀ<N|c'í…@^owG?ý¥óå?ŠZ?´åp‡§~µ?«Û^¸r?öÖ»cý@]–ý]
¿àˆÊ>}¿ãš:Þù;¿à›T\ÈX¿ÐÜÍ`pƒ ¿áf¬ƒ§À¿ê†#À¤ukAGNbll3FGL J1209.4+4119B3 1206+416?ïý†ß5bÁ?$?"à¨O?3Émõ?$?"à¨O?ïõ»›¢|?TTGªŒy¬?TˆÈ»ñj?TTGªŒy¬?ï÷^©·&¦?T±¯'Eè?QB¬'²´7?T±¯'Eè?ïà8+}¨?WRtÏh¿?oÇÕÁh:?WRtÏh¿?ïû¦ãf±?4ˆ.hJ*q?Ag¿ãu|Ï?4ˆ.hJ*q?ïÚ±ð??vd{"2ÌZ?rñ§&9ð{?vd{"2ÌZ?ïìékz2²?uUIÞÚR?c"YÒMý?uUIÞÚR?ï¢}ÿgÝ=?sË+%âV'?‡`€¹Üë?sË+%âV'AGN4FGL J1209.4+7608?êð¿P•ø-@D\Fà!qÀ:¼¼Š_ióÀ<Ön%wˆÎ@ÿ˜Î˜~ç?üñÊ,ß\?ʃ2yúÂÔ?Ói¢À^Õ@YíÚcŽE@	PålU闿ìëF…¿ºõ¡Aٔ0¿Û·yT¼¿Ü_G£­™¬¿êñ0š¿ïÿJ-J»æAGNbcu3FGL J1209.9+76072MASS J12093020+7609120?ï÷	_¶Z+?QVˆ»œ??Qí@ˆLêe?QVˆ»œ??ïòfàt[?YxÜr¢®?[3æZ"*'?YxÜr¢®?ïSŸoW¸?‹"{VöLq?•œì¥m	?‹"{VöLq?ïÒÜX°ñ$?WiQI+þ?v'Ó°viç?WiQI+þ?ïôù߁ë?SÃf$¬Çœ?V@ă	°?SÃf$¬Çœ?ïÑâA9ln?v9«AìšW?wßW›Ô?v9«AìšW?î^¦®R?ž™éŸ[ô?ªžÆÖÈâ?ž™éŸ[ô?ïpng'´ž?zã$¬wŒ½?'ò3žH?zã$¬wŒ½AGN4FGL J1209.7+2548?Õ½¯"hé_@T%sBí»ZÀ;|iÃ8èÀ<Õªøg…@1<¼ô½'@9±Y©¿'?ÑŽŸÀz.?»G‹.ò±¹?çÀÞöÅð@Ͼj´SÚ¿ïé‡þ'•ê?ïÏ[½•ø$¿Ç÷D…(0¿Ù·ª%ØØ¿ä?"=ßßy¿ïñ/DÀ#AGNfsrqB2 1207+26?ïýªu^ü»?+NÖIô¥å?2¬WÇ.x?+NÖIô¥å?ïðB™0=?^º&…¼t:?_zäI®†N?^º&…¼t:?ïêKe5†?d–¨h¶m%?e´ó¿æA‹?d–¨h¶m%?ïÙhÔ!LM?XÚ²¥Ü*?sK•ÓÜùz?XÚ²¥Ü*?ïý²Ö+›9?+Pš-øÙ?2iMó:6=?+Pš-øÙ?ïÅ]Îx"²?'­=9Ä?}Q¯þþ?'­=9Ä?ïßM£
?y´
c§3?pYw;®ü?y´
c§3?ï_ä}Ý??ƒÛ©(gÙ?"pDX?ƒÛ©(gÙAGN4FGL J1209.8+1810¿é¿T¾•žÛ@S9,{‰
ZÀ9•8¬øÀ<IwëÉè@&ãÏGÑP@'ìB³Ù·?°–1Só?™6&`D–æ?å—4àh@i$ ô+á¿Í{.I"s•¿æD}ˆkõ¿å¹î£·*¿æe̽ÞGt¿èvuþ	ῼß0Q¬pAGNfsrq3FGL J1209.8+1810MG1 J120953+1809?ïþÙÊa7¨?ùSˆˆè?"c[:ÅÞh?ùSˆˆè?ïöïýö²Ç?V(¢iل?R R°?V(¢iل?ïòó{üêf?H‹ ÑÈ1š?Z(´?H‹ ÑÈ1š?ïÿlõKÆþ?þl1{Ê ?aOB$'?þl1{Ê ?ïýÕPÝp½?,#/~-‰?1UxÄ6oY?,#/~-‰?ïÖaÊåì?ëÇÙYã?tϬj÷?ëÇÙYã?ïè²Ð¥ø?nÍ·K•?gM0$Uæ?nÍ·K•?ïþ߅p4?E÷±l£?"® ÌGƒ?E÷±l£AGN4FGL J1211.0-3800?ÝÔ·Ý|rl@8,aՈÀ:`~XËs0À<b$Óš@ð[Œm·@¶ûú·Á£?Â1²)³W±?Á2Ã6K¨?ÿ"Sd+"Ã@ð™§0†?ä±+¡nz1¿Ò·6B\Eü¿å;ÔÂd"¿ÞC5ߵݝ¿êðj`Æê5¿ïó‡K¹;öAGNbcuPMN J1211-3754?ïúnió9?;ùN^‡O•?FG‰PQQ?;ùN^‡O•?ïî éÚ?`qnw—ê*?a_égŽ¢?`qnw—ê*?ïÜJ§ ÉW?p}p™Ê.Ë?qÚ¬xŠPŠ?p}p™Ê.Ë?ïãvzŽD/?M7É!c??l‰…˜7q??M7É!c??ïæ<ȻΫ?eÜQ¤¶Kã?iÃ7tKÜk?eÜQ¤¶Kã?ï»Á.³ò‹?ˆ¬·fZ¾B?´cÙs?ˆ¬·fZ¾B?ï´æ©9A7?‡êÌIìž~?'ÆUºž®K?‡êÌIìž~?ï†g×:ö?t|_äüuZ?Žf
1B~f?t|_äüuZAGN4FGL J1211.6-2735¿ïõ%W8²4@A: _ñØÀ:?d?D¹mÀ<‹h~n›@@ï3@WM>w4?Áï$»v8A?²j(gÓ"ý?ïˆØ¡lKÙ@
©;×òp?¬˜¾A2"¿éµ\8;¿æçKžd¶¿æ—4d‹šÓ¿êoÔ;V¿ïþ§¥Ë×AGNbcuNVSS J121135-273615?ïúæz•>ã?Bƒ¾Ÿ†e|?Df"?Bƒ¾Ÿ†e|?ïô¼ëXS(?W£Ã<uê!?V†)áÏ×?W£Ã<uê!?ïåCœjŒï?nÂ>À»_¨?j¼có°Ã?nÂ>À»_¨?ïøÚæQ>r?44¿îaä?L"fûX€M?44¿îaä?ïú3õûÅ3?@ëüg†p¼?G0'uV3?@ëüg†p¼?ïÎÜ{/e?uz³¤V'Õ?x'Â|ë!Ç?uz³¤V'Õ?ïáæLÙ*1?vñw[-?n³?'þÿ?vñw[-?ïÚRYÇ¥#?aû9áfü}?rÖÓ
¿r?aû9áfü}AGN4FGL J1211.6+3901¿Äù,B9q¢@Rß`þG™À;Yá'nÀ<ÞÖÜGª@î',èÁJ@ƒœØ{?ŔS»d¿ª?ڜªVf?ä UàÝ%
@-=ÐÆ?ïÎá£0ò¿ëbS².»Õ¿ä+z!"4-¿Ùô¼ .ß¿Õ'äKn"\¿Ýõ3ô#RëAGNbllFIRST J121134.2+390053?ïþZð«=?óԕz­?*Pô`âlþ?óԕz­?ïø9ê~ÛË?Q[øčfB?OUU1"ˆ?Q[øčfB?ïùóçBï¿?4Ê;ÔÀ¬Æ?H0c
Šñ­?4Ê;ÔÀ¬Æ?ïûÍ)œ?+°±BÛõ¶?C¤Ì]–˜~?+°±BÛõ¶?ïþX–L»£?Ð]s/ׁ?*v™:Qø?Ð]s/ׁ?ïßIŠJÉ?q
\
?p[;	HW¢?q
\
?ïûTüuu½?I+Íð'ô?B¬
–FªÈ?I+Íð'ô?ïçd‡áWÁ?\‰réWK.?h›xJçx?\‰réWK.AGN4FGL J1212.0-2326¿åÔ~.?j@CDQ£"îÀ:_bnŠ!WÀ<N>Ȓ«i@ ²WlÎ_t?ü‰ý_;Ϻ?Ĉ°'Ð~ˆ?»ã8)‹À?ùÎފdrp@	³l`%…?â}E`1n¿Ýy]¹ïz¿âLuĨ;¿ÐàØóK½¿áƒè¢–Bw¿ÛX£Ó¯AGNbcuPMN J1212-2327?ïÿºã6?
üLp¸O?ˆ¤úëf¥?
üLp¸O?ïòÍ¥9àÌ?]®¤
?Zdµ~÷W?]®¤
?ïöŸâ!â?fÊL9jM?SÀ"²:¬?fÊL9jM?ïøæ¨`?0µÈ•_Ÿ?Le`RVh?0µÈ•_Ÿ?ïÿ•¤¨¨?%õª?MGˆõ­?%õª?ïÎ<QG£á?{)irq?xá×}*O@?{)irq?ïö@}Ú²?j'읹?Sÿ>
¼?j'읹?ïêÙ|!}m?Q½ ì•†7?e&ƒÙ3?Q½ ì•†7AGN4FGL J1212.0+2242¿°Þ©–'\@T½D¦"À;1	G|À<Ã"̳¢@‹F©\°/?ÿw_²íþ?ÆòT†?Ï?³ˆÝðǺ?ëöŸ™Û@ÓêÎ?"¿ïÿE€Þ$?ïö?ŒÝÉt¿ãI=Š¥
¿ËÉKãÙ-ٿꇥïaL¿×+¢zé«*AGNbllRX J1211.9+2242?ï:*ì?¹ ãl™?Œ>¹î©#?¹ ãl™?ïë»l8?cÀj«{ä?dùùWїr?cÀj«{ä?ï±ÜPšÅ?"=>h]Cø?ƒ ä¢ è?"=>h]Cø?ïÈ"Ö­»?ctí"Çí?{ö½™x–{?ctí"Çí?ïñC½€:?\Aæê"<–?]ùx5Hœ´?\Aæê"<–?ï¨[š@ħ?'•«vŒ"?…éoÎÖ#?'•«vŒ"?ï«L£¶lÓ?†A¯_Å°?…,×…"T?†A¯_Å°?îü¿31/Î?'~íÆÂqª? 4É}g(?'~íÆÂqªAGN4FGL J1212.2+2442?ï¸ØPÛÝ@T6éNã'âÀ:ç{³Õ…À<¶tðlå@?EbŠ¹­?þñ
‰U~¸?ÉL'jPUÙ?ËÙ@x–Ó@'åøí½?þkÌ´Îÿ,?ïŽBî's¿é='þ¡±¿ØëxßdÔì¿ì{Ô!Tä^?ÐZ"ŸY¢¿ïþ"ØrAGNbcuNVSS J121219+244130?ïöÕ[ÍÂ?P'hæzö$?RàU2fû|?P'hæzö$?ïÊ:•küA?"Ú5]=?zâµLÁX?"Ú5]=?ï¡6âGæÒ?ƒ|mi—?‡²GxUn?ƒ|mi—?ïà(ŒÑ	?`_ôurôÅ?o×ôEÔ÷?`_ôurôÅ?ïØWÕ~ø?sÅE©¶Qö?sÔV~‰?sÅE©¶Qö?ï(ì
ëâ"?¤areìü•?šâ~D;‰½?¤areìü•?î·8[?*³t3ú?¤Œ~~æ.?*³t3ú?îùæ¾K¼?š&
Fy
? nñ"?]D?š&
Fy
AGN4FGL J1212.7-1402?ï»|8Æ×&@Gã1üÒNÀ;lk§îÆóÀ<¦®òÇ2Y@ ߪG;Ô?ÿø¶zzða?Í&"©x3î?^ô¼kZàÚ?ý©t"$à_?ïŽ:ºæñ¿Ö¾"š´¡³¿ïÐéÅ?áý'aĖ¿ãˆŸvRl´¿ÞØ⚔kAGNbcu1RXS J121240.3-140141?ïüÜnQú?T$gômì?9ðK?T$gômì?ïðXxo°ñ?`¥/ S#?_Oªk¢?`¥/ S#?ïê\)MN?cóҟf?e£€–
§?cóҟf?ïöhSÈÌZ?@º&C—?S/XòXLE?@º&C—?ïúëقgÏ?@sd{uÔ}?DPš™§Íž?@sd{uÔ}?ïÇpÏBjU?'	qÇÜ5À?|G˜)>?'	qÇÜ5À?ïärüuŠ?r!I›m?ki-~?r!I›m?ïÊb[·-K?r!Ç|™—?zÎÒ9Š?r!Ç|™—AGN4FGL J1213.0+5129?цˆÈï{+@P%˜Çâ'AÀ:jQ•ôÉkÀ<°!èˆ6@aþ÷KÑ@pÛ4n?·<? |LW¿–¢÷Äг?Ú¤ÐÚN@ýŽøUç"?ïDž/IŒ¿æq*_Oð¿äÊìB3]¿ÙûÏdÛr¿ã@TN5íù¿Ù"-Qqâ›AGNbll3FGL J1212.6+51351RXS J121301.8+512942?ïú£Ñ;M?8ºXé#f?Ep¼ƒ/>d?8ºXé#f?ïöo2'ÏP?T"–Ø?S!š^¯p˜?T"–Ø?ïï&è»Ú{?jàÝné>^?`Ù"¾,¬?jàÝné>^?ïà'x¬d?Vg%ôž\~?o}äÔ;æ?Vg%ôž\~?ïó÷ʍ"?PJkÝz2?XjƜUç?PJkÝz2?ïÜY bê?qÞÇãa?qÓ/ÓZm"?qÞÇãa?ïðþa^-¢?ný·ðÄ?^=Â\+?ný·ðÄ?ï—ƒÞ­†?tH€Ä­æÐ?Š>Ÿufƒ?tH€Ä­æÐAGN4FGL J1213.3-2618¿ï&‡]yOD@Aãƒ'gMÀ:gn³<À<U£Ô…þ²@!(GœÌª?ùmóXQЭ?È÷V¹Eë?ÌÁïy%µ@@~$É
%@ÿ¤åÄ¿ïÿî' Ç?ïÿÑa\w¿ÝÇyB=?)*sqäT¿á…¤O\_¿Ù+¡ƒóÀAGNbll3FGL J1213.1-2619RBS 1080?ïû¦r"ºÉ?:¾àÆÝA?Af7u¡š\?:¾àÆÝA?ïê¯Ë#M?c¦Ä†?eP4¤ŽŒ?c¦Ä†?ïÜÓ_ãëL?s3ԈJï??q–OõM)í?s3ԈJï??ïã÷›,—?S"'ãª5?lø<÷ñ€?S"'ãª5?ïòæcÄ?Yyô^FgZ?Z38¼Š	"?Yyô^FgZ?ï¯Ê(`Nþ?Š;¾Ek16?"
u÷
ˆy?Š;¾Ek16?ï–C''Ò`?‹€>'0l;?Šo›ÛËë?‹€>'0l;?ïNéáÊO?{¥*1"ïØ?Œ¬E}>˜b?{¥*1"ïØAGN4FGL J1213.6+1306?ËïØñÚ^—@R[Ÿ@¢‡À9·ð†nDÀ<.z>å@mï@Ec#»Æë?¶oè›4y?Èì$+@Ž;—…Ã?û,;rFïS¿º)ß!Ž5¿à_¾ÿ"°¿ãΈŽ¯Z̿ꮊ!V'Ý¿ç"ñÿ·/Ø¿ïþàEO•jAGNfsrq3FGL J1213.7+13064C +13.46?îBÍƃÞ?«VÙ¯?«Ó#•:Í!?«VÙ¯?äùƒ˜6©F?̍EBªI•?Öøϒ­u?̍EBªI•?íÊA†vëÞ?žF2´ö?±­óÎo
?žF2´ö?ꕁT†ó'?©d+ÀÒ?Å©ú­ä1÷?©d+ÀÒ?çcYô"g?Å5GVçÔ?Ñ9LÙá2?Å5GVçÔ?Æv†#?Çή%}?ê~¢^}þw?Çή%}?æ/T®zs±?µ'¡0q?Ó¡V£ž?µ'¡0q?ÐùÁX`¥m?·ËoUëri?çƒSÏ­I?·ËoUëriMIXED4FGL J1213.7+6423¿ç*PÕ@J9C¬ÅÀ:¿ØCùTÀ<ȍÿ1£ç@3ʗé@K@Y|´†…?¹:üUP"m¿±™Ö?è"i?ö'ÄãÊ?T@
«‡WÎ?áM̧
£¿êŠ~¬-p¿áÌs`ŸÒï¿äÏ:eV›î¿íOÐÂû'³?à$"3ÿAGNbllNVSS J121348+642524?ïûºŽ0Ú¾?Hð°ù?AÇßÜo?Hð°ù?ï÷
Yž›¦?R|€qèð+?QåL™d•?R|€qèð+?ï·|	ª'?'T÷¸§H?' ý¡
-?'T÷¸§H?ïöû"¶Zð?;›»Î}?RÖgOp?;›»Î}?ï÷wÌ"?RZxNC?Qh&0ˍ?RZxNC?ïÚ«fíí%?söñ4ÊZ×?rªLg]A…?söñ4ÊZ×?ïÒÖÃ4Œ?~OEq\?vý"'èÙò?~OEq\?ïÇ[󊕊?j±äS#+?|R.V£O?j±äS#+AGN4FGL J1213.8-4345?ìlL¯!&@2—àXšËÉÀ:Jr}ËÞÀ<%)Wèb@ÚøžaÕ]@¹cc}?Ä[ãÁn?±Ó)]F'?î0kؖ/?ú¶[
í©f?ïðØïÿ¿éÄÌîZ¼¿á6sŸ_l¿ä‹«šM¿àb‹"¿ïÿýawAGNbllPMN J1213-4343?ïõQáI0¡?HÃv	Ÿµ%?U\=së?HÃv	Ÿµ%?ïÀ(Š@hÙ?'±à`ö‰?ëºÞk»O?'±à`ö‰?ïÚ\ ûô¿?nðߜJ]x?rѯiø\Â?nðߜJ]x?ï›Çë«N?lÈè¦ñë›?‰
ݧÜ?lÈè¦ñë›?ï指És¸?`V^™Xû?isxA‹×?`V^™Xû?îÓFêRÍ5?¦ûè\4I?¢Ë'X?w³?¦ûè\4I?ï  É[®?‡ƒÎˆ4?‡×Ͷö"~?‡ƒÎˆ4?í Â'Æï=?Dh%2ˆv?²ùëèìŸ?Dh%2ˆvAGN4FGL J1214.6-1926¿àIÆÖqCî@EJ8Ÿƒ¾fÀ;;÷'À=¢ÌHB@ài4!Ö@€\FQóé?ؼ‰ˆª^
?ïÿõ^'@ÌiegÊ?ù…hŒ,¿ïšÇ‰W'?ã¨	3…hŠ¿Ö‹¥»ç¿îD´š¦ßÓ¿èB½—¥¤¿ïÃㄟ6'AGNbcu3FGL J1215.9-1926PKS B1211-190?ëQ±€¢?ÄB¢OSWô?¹9ÿÍw?ÄB¢OSWô?áÞÕ*¥Ï?ÊÏGÞ2r:?ÜBUÿª´c?ÊÏGÞ2r:?é•×`W6P?°˜à"h?ɨ¢~£&¿?°˜à"h?á.*¥›©?¶¦zâþ?Ý£ª´Éö¯?¶¦zâþ?äÖÛó ?јg×÷ð‰?ÖRH¿áÏ?јg×÷ð‰?¿îÕ?  Ç¾Î?ì?Å_<ž?  Ç¾Î?ä')í h?¹nª;ÂÍ?ÖÛŬ$¿0?¹nª;ÂÍ?´'vvm´R?¡iTŸ—ôú?ío±0í'F?¡iTŸ—ôúMIXED4FGL J1215.0+1656¿æM˜Åfڈ@S2œ#·•-À9x™sÙìpÀ<C?»òn@ÿ¿¼îÞE@!	!ç±U?®ôA¡?Ÿ|æ
C?êêú~Ù@'³{"†¿Ð/Ú¹š¿ã ^l¢¿å-¿öût€¿æ,£ÌùBw¿é•}
Ú7¿Ôe™¢Rû¥AGNfsrq3FGL J1215.1+1658TXS 1212+171?ïþKea·3?¯%C¿ì7?+I¬fª7G?¯%C¿ì7?ï÷=
Ò{?UJMý?Q…ädÐ?UJMý?ïïpe:8Ø?NÄ ?ã]?`š™Ì'â?NÄ ?ã]?ïÿ¨,bK>üŒÚw¬Ï?ôâeÚó»>üŒÚw¬Ï?ïý}'¹é?+-ŒÐê[?4iXEHý?+-ŒÐê[?ïÒ%\Àd?‹¸}U-hu?ví~°£Ž?‹¸}U-hu?ïéü@ø©?j×Ȏ"©§?f¿ãêO†?j×Ȏ"©§?ïÿ}פʮ?	SÄóÿ"?Eµÿ›&?	SÄóÿ"AGN4FGL J1215.1+5002?åLéâ 4î@PƒcÜHjÓÀ:†…ÀŸÀ<sŠƒ| ã@ !¬zúÝ?ütA…ÜMs?¹ß>>?³kAþŽL?úâ$íö@@	f†ã¿ë…e?IìÞ¿×f'|E˼¿à.jáö)½¿Ù~˜¡ÌîׅܿÜz>à¿è~ú1‰æAGNbll3FGL J1215.0+5002IVS B1212+503?ïüŠT#»?/¢'nÜ?;­`ê7?/¢'nÜ?ïñ
áWH?[koÏð'€?]ê=c`Ý?[koÏð'€?ïé@Ä/3?mÕkÀb7?fo¿7±DÎ?mÕkÀb7?ïſö÷?b0îeõçq?} ¾ô'?b0îeõçq?ïõ+§½b?MHõwí?U¨°ó.^®?MHõwí?ïÊf½Æ–õ?y%äÅ)ÓÙ?zÌ¡5%z?y%äÅ)ÓÙ?ïçb¦ÿ3?tUgµKÉÔ?h€mžu?tUgµKÉÔ?ï—ÆŸzô?ˆ"+Lˆ9?Ÿ­2ïÙ|?ˆ"+Lˆ9AGN4FGL J1215.1+0731?Û±·UŸÍC@Q%¼¾aÏÿÀ:œ¥ÛÇ;"À<k
€òç@!OŽ%óÃ?û/ã7r]?¾9 PB
?˜0':±š?Ý-o|@5ÜiM¿ï¥˜Æï¾?ïã€}"Ô‰¿ÝXcg™¿Æð»ix¸¿äw,ò§Q鿾yĒÁ³AGNbll1ES 1212+078?ïý»Ök˜;?%1+øç!'?2!Lëσ´?%1+øç!'?ïòæGOÓ[?\Åñǜ!	?Z3q§Ñ*?\Åñǜ!	?ïô3:ŒeK?G>¡<wR?W™Š§üšX?G>¡<wR?ïïžqMRÍ?I»asÖ­?`aŽ Ï;e?I»asÖ­?ïúlŽÃ??"W-՛·?FOﶲû¢??"W-՛·?ïˉ×Þ?€|ç°s'Ù?z;pS!,?€|ç°s'Ù?ïö¿miñ?[Ù¢D¹?R%XxíË?[Ù¢D¹?ïЗG¸Y?j£hx!?w´\‡,-?j£hx!AGN4FGL J1215.1+3513?ވCœs#õ@S³Q¬šþÀ:׶6ˆRIÀ<–µI"ˆÁ@Îbÿÿ'@<ewS?Æ¢
S?ºÝzÐj?ð#	"ãÿï@lÿGµ¡?ïýl!'J@¿äž‹`Æ¿B¿èúàŽµ:¿ä îzÔ]¿ïø½KO‰«?éÓÈ3àØAGNbll7C 1212+3524?ïù6fT¯?Dÿ߈ÿmw?Kã%h°Œ?Dÿ߈ÿmw?ïìÈ(*ôÿ?k[r×·Ü+?c7×óG'?k[r×·Ü+?ïÃje5?tÍú]?~JÍq
¥?tÍú]?ï½<âð‹Õ?iÒ¯†á<?€°ÇM{ò¶?iÒ¯†á<?ï÷ÖjEª?RkŠu`ë'?PS+|C*?RkŠu`ë'?¥Šú¬?~Ÿ;pβ?‹"֏'å.?~Ÿ;pβ?ﲯäš?"cŒ:å?ƒTð蓅?"cŒ:å?íÀ>ý¸? Rìн(?±ÿ>˜7Á? Rìн(AGN4FGL J1215.8-3732?ïµD@æû@8ˎ\NµpÀ:ØxFÜÀ<h)à¤&@o›Cgß@Ö¢óµo?ȕè41_ô?²
M`Ûâê?ë%ˆ M?þùr奶³?ïÝÐË_ƒ¿åä¶Î]Ç¿é®`Ðû0¿Ýgzbœ­J¿ÓK' Q¿ïþÜIA'rAGNbcuPMN J1216-3734?ïûlktSu?5vždt4?BNS0×?5vždt4?ïê§Ó©?j¹õ‰ÎX:?eâX3&À?j¹õ‰ÎX:?ïì	ŸÕ·œ?eýé-`J?cö`R#Û÷?eýé-`J?ï	"¨?E»²ÒJâ?`_b.ÔïÓ?E»²ÒJâ?ïú©®(‹©?>¢¿Ûw?EYH/FVë?>¢¿Ûw?<}gg?ž]DԛMN?‡ž0à¦&#?ž]DԛMN?ïìp^G?j"'8¡X?cïâQŸ?j"'8¡X?þ¢T?€ê‰ñ7ë?Ž—»Ê¦>ß?€ê‰ñ7ëAGN4FGL J1215.8-1733¿ÚKDc©•@F=Â;yRÒÀ:F¼—Ëc@À<H…7È@N´©‹Ó@ú0bžZÉ?ÂÛy¸Ó›ž?³Ffdÿ´?uøª¡@—EôÖ×?ïiæþÒ-Š¿ãã
ìQÍR¿æDڐå×ê7@Þí¿ïÿèþ†®/¿íÈÔàl'ÏAGNbcuPKS 1213-17?ïóŽÎːÉ?aÑØڊ;?Xâb<ãn¥?aÑØڊ;?ï㙆4ž)?m}žá«ü?lfyÕ¿m?m}žá«ü?ïÑÿžÓ?sÝhù¨ ?wx0–9­?sÝhù¨ ?ï­+÷•?o wÖ¼"å?"¼õ9ÚÜ?o wÖ¼"å?ïéÎìÞ´?aÔim³?f1/G`?aÔim³?ï¤èz'cq?…œdªÍÁ?†Åá€u÷¢?…œdªÍÁ?ï´0:Ò±5?"jÌ"=!¶?'óñICîÕ?"jÌ"=!¶?îM'™dy?•\ê"0?«&ÖlS}e?•\ê"0AGN4FGL J1216.1-0242¿îõÚx9«%@M{›€#¦ÎÀ; ÆÞvB|À<›'–FþÂ@ Ëÿ)@k*?þobð ?É'dÈ×tÆ?´¾¾l6à?îcâÞ1#9@Y‡¼ÍPU¿ïÿZ=¹?ïêâ—9m	¿¦IøŸ¿ä|â((¾¿ÄŒùM3e¿â=)¡dPAGNbll1RXS J121603.6-024302?ïýÊîÑ.†?O&ºXAÆ?1¨ˆDáÂZ?O&ºXAÆ?ïñÿo?­?cÑí¯ù‰?\!|uF&?cÑí¯ù‰?ïæBù"™?rYÏ‹Hâ?i½`TÀ?rYÏ‹Hâ?ï÷4âgz??ÎÜwK<¸?Q–ãÒ¼ì«??ÎÜwK<¸?ïý"$Ãô?3ožñ䳚?6îؕB)?3ožñ䳚?»'š?ƒi…nçÈ?~³ ,î?ƒi…nçÈ?ï卅<j?w§W{öž=?jrå¨mX?w§W{öž=?ïڕ0íøZ?h4v¢ô48?rµg"4^Ø?h4v¢ô48AGN4FGL J1216.1+0930?ìh-èèٕ@Q Õ{Ç÷{À:bSåZbÀ<|ërl.@ndD"D@#~Ýx?¼aU"9]?ªþ8C'$¢?ð×*à¼?ÿ†k5X'¿ïð'Úb·…?ïS(Ü¿Þ¨»àì>'¿ã™Á§Õœ¿äƒ×ûÔø¿¾éÀÎfÕÍAGNbllTXS 1213+097?ïû(ÂìÏ!?6莀¼²™?C\ó[øx?6莀¼²™?ï獑è9)?lW¯%´Oì?hrn+§6?lW¯%´Oì?ïä]Õ¼G?iT-ªÇÖ?k¢*Úř?iT-ªÇÖ?~3 ?gRÿÓa?€˜y#N"?gRÿÓa?ïð!,†­?Wn}W2ݞ?_é½ÍnEø?Wn}W2ݞ?ï A²¨?¡š´~?÷Âà3?¡š´~?ï͍¦`X?~§äUµ€?y9,ٔ;Ð?~§äUµ€?î¼íD¢­{?"Ñæ`Htv?¤1+³AsX?"Ñæ`HtvAGN4FGL J1216.2-6121¿îÖèæ͘¾?ó˜2ü¬ŽiÀ9Ü»‰®jÀ;(};•"@•þYŒ¹@͒Z
7'?Ðùn
Áà?Û¯žS<½ö@	¿v¢ôŒ.@ ÂèóI?åmíät‰?¿á}S³{j¿áÓçþ×`ú¿îO
`;¿âzm"gÙ-¿ïà‰B37AGNbcuPMN J1217-6113?ïY;KZœ?—'³`d?"Ýx"%z?—'³`d?ìnq­l_O?ºhqݬ²À?¼Œr"Š?ºhqݬ²À?ì¯p@¸_‹?¤³IŽ*Ò?º"}ú=¨?¤³IŽ*Ò?îiJ0Xk?‹p£0'?©oû^²GM?‹p£0'?엜–ú?¸p¢)T?»CH/ï‡?¸p¢)T?ÏÀÑÁÔ ?Êi(ß-ˆ¶?è:ËŠø?Êi(ß-ˆ¶?äi_øì˜ù?º­»W¸k?×-@&Î?º­»W¸k?ޅšÁbX?À^Öɔ¢Ô?à½2Ÿ~NÔ?À^Öɔ¢Ô	MIXED4FGL J1217.9+3007?îǍÑB@Tƒ×Ûô‡ýÀ7ÔÄèÒ½À:ÝgD²·x@ýpÌÚ?ýªˆ>•g?'H]+?§¡—s¡k@6ï^Èt@Δ$9Æ?îg¬sßÌ¿Ùù{Óë¿Ýç‹z‰‰¿Þs¨£ø˜-¿áJ'Á¿Þç=[«!AGNBLL3FGL J1217.8+3007B2 1215+30?ïø_S¼Y|?T!šé'±Ø?N'±²ú'Ë?T!šé'±Ø?ïòž4«OÇ?aÿL"¥'?ZÖ8­BÞ?aÿL"¥'?g¬¦V?‹§~Fld?Š^&ÖjŸ?‹§~Fld?ïû1!ò)?6/¬EËg?CÏ<?ÇÂ?6/¬EËg?ïüf2d[?5Úœ?<Îk¤mÙ¼?5Úœ?ïË-êÁ¹?ƒÚ»ñßá?zi
Ï£q?ƒÚ»ñßá?ïÓ_ÚAe·?ƒh29Õ6?vPÏ~ðƒ?ƒh29Õ6?ï÷Í
íß?E†Õ+Ó»¯?PeÕÀèó1?E†Õ+Ó»¯AGN4FGL J1218.0-0028¿ëß4¡ÐÓ@NŸa»úìÀ9ûKиê˜À<0=áÄ@b÷Æöt@26 M}a?»®ÌÒ|å?¸`ýµ'?ùhöHÇ/@	i
؅½š¿éã_•'Í?ÁríÒ¹K¿å^ïäÿÉy¿çՍ@öv¿Ú">þî]¿é¹¡KêAGNbll3FGL J1218.0-0029PKS 1215-002?ïþ‰ÑX*l?%:¶M‡Á?'bíÃ--*?%:¶M‡Á?ïòþ6?cJ»:?[éĄÊĦ?cJ»:?ïð5¥(n?^՝A<?_"µàžO/?^՝A<?ïöžëVê?;utAñ@?SÂÁµßKÞ?;utAñ@?ïûø¸§À"?8"b""!?@·ÓJ?8"b""!?ïÄÉwq•]?Œ™Ä?}›Deqá$?Œ™Ä?ïâ@kCߘ?s±šccg±?m¿"«¢H}?s±šccg±?ïÇxÇçà¤?m³«ç±ä?|C›ïâáï?m³«ç±äAGN4FGL J1218.5-0119¿ïkšÍm¨ò@N;gäçïÀ8ÞÚVùÀ;©É™;¥È@p¿#¤@-;¢m}²?¨n'>´Ï?¹3©û'†P@À2˜À¥@ÌÒÖüü?ìïÀÛå¿ÜÈ¥ߙX¿áéÄ[å¿áb©B"	¿äës`¿çôþÅwAGNbll3FGL J1218.4-0121PKS 1216-010?ïü8«®?4œ}µÉŒ7??¾:,eZH?4œ}µÉŒ7?ï﫪EìÒ?dÙÙÉ7?`TUµó¦-?dÙÙÉ7?ïæ[Ÿkž<?jW5R¾…	?i¤`oEûê?jW5R¾…	?ï÷­C°*?8U²ë
Õ?P¥y'æ;§?8U²ë
Õ?ïý^ŒA0;?,319?5Ÿ2
{,?,319?ï±\ªr§?˜8½n‡ˆz?ƒ¨ùG¤æF?˜8½n‡ˆz?ïãŠ$%?{[·Þî€?luóüÙ[Y?{[·Þî€?ïåÑ
¬Äw?Uý aÕI&?j.ò"µèu?Uý aÕI&AGN4FGL J1219.0+4827?á	‰œ@Pñ<64À;d‰èK®TÀ<¾©Ü¡V@àÕ:Y˜"@](¯Fª?ȤvçvF¿Š­ükå›?‰ö­›Ú@išÎM?ï`¤&ó¿æBnd!¿ê¯s?è£B¿Å
GÅwÄ¿ãît½A>¿ïÿf¢¡U%AGNfsrqON 428?ïüæµM¡–?2¶
@'S-?8ÊT"ù€?2¶
@'S-?ïø7a?OÓ&nƒà?Oï#+Û¨k?OÓ&nƒà?ïÏ9šð§?'N0Cýv?xc2zᨓ?'N0Cýv?ï÷>û½È?7 ™¶X&y?QƒáøO8?7 ™¶X&y?ïø²ÜË.?MÂS×­xa?M7ƒ}>÷?MÂS×­xa?ïØJxõ?w՞ùo?sÚÃÐbÐ"?w՞ùo?ï¯4
MÆ\?‰H"ç2??"2üŸ×Úö?‰H"ç2??ïÐ@/e?gáÚõ]Po?wßù
¥v?gáÚõ]PoAGN4FGL J1219.0+3653?Ûò‹ø
,@S…/D')‰À;oP–À<Îâ*,#t@nx‹¬ñæ@©A­Iz?ÓÀQ>a¹?ÖÇö8Öá#@÷P™u‡l@B8!°º¿çt]î$?îo^‡ŸÇ¿Ù£½l²†¿ã2HQ¨i@¿ïûñH¿ïë6ÊñUAGNbcuNVSS J121915+365718?ï´[»"çr?€•ÅêO}?'é=Íeƒ?€•ÅêO}?î'ÿ:×?©Ói­"¸?¦à[ã=˜?©Ói­"¸?îkhé?•
™Âülâ?©I~ôÄ÷?•
™Âülâ?ìÕ"õß{â?œÔÅÔ/ùŠ?¹VèP–-o?œÔÅÔ/ùŠ?ïb˜n©ßk?ó]àNíu?"¬ò%œ¨µ?ó]àNíu?ë$"қvq?ÇáéèD*/?Ãotµ'&;?ÇáéèD*/?ì'?Žœvª?¥ˆ¨<—†?»î‹J±?¥ˆ¨<—†?ãÃ"X?»+‰›Ÿ®1?ØyÏ»OÝõ?»+‰›Ÿ®1AGN4FGL J1219.0-4827¿àBÁ ô¬»@,#ÿï9_À:+3ªQwÂÀ<>J—ÓƼ@bxqÏ{@¹m	Ö¶?¼jgÒÍõ?ÊULù	ð@âÑ¡GãÄ@ï¾'˜uW¿ì	ì³!Ÿ?Èx¤&æI¿áå¢áìď¿àÆY`nº¿êÁ¿åԐ{æ˜AGNbll3FGL J1218.8-4827PMN J1219-4826?îVXäjÇ?¬ÉçZ»º
?ªšq»ò"?¬ÉçZ»º
?ï6Œ›A?™Ší
X>H?™.lŸÇxS?™Ší
X>H?ï-}jþ•a?'ÈrÖÿY&?šPR£œïé?'ÈrÖÿY&?ïoÉ,?pƒ~°Ð9?'Ú~ü~?pƒ~°Ð9?áLú°›úÙ?ÌÿþŒ|>"?Ýf
žÈ
N?ÌÿþŒ|>"?é¼"tbí$?Çï]?#M?Év.tKp?Çï]?#M?âS+3"?Á­Qƒ§S?ÛY©˜Ùïå?Á­Qƒ§S?ëLÔí¶/?§@ÀámÁ?Â̬I'Cï?§@ÀámÁAGN4FGL J1219.6+0550?æcÓKcx@PÙ¼¾aÏÿÀ:êÒëʾÖÀ<–"
>@XÜüŸÜ?ÿ'ø½ì_9?˼#.XX?•_¼~?óF«ë«µ%@E9ÜœH?ïÁCâWùf¿ä.y$¯ò¿ßõ]¨)¿à{Áâÿ2¿äL-4ìp׿áÿÅGAGNrdgNGC 4261?ïþ…bf7Ô?âk39¿h?'©ØªžH.?âk39¿h?ïðcÛ¥5b?c,@á(ÇÈ?_8HJam?c,@á(ÇÈ?ïöñnËBg?Cœ"y&p?R"Ó?Cœ"y&p?ïëمܒ?G:2ZÛ8?dï&d%íó?G:2ZÛ8?ïýK¤?/ÂÒ³?3ßQˆõ?/ÂÒ³?ïÂìÎ
ÙK?ƒtCx?~‰˜ó"ú`?ƒtCx?ïðŠ‡‹'³?d©ZXÒ±?^êño«Hí?d©ZXÒ±?ï±\V(g?l¯tUGA?ƒ½èçJL?l¯tUGAAGN4FGL J1219.7-0313?»«Ó\LËÏ@MYµÜyÀ9õÍXãÆäÀ<7"U²¹ü@ Æ2ÿ±§?þL(²¦°Ù?¸DÛ&VÖÑ?§(ÍÂ?ñ
ÿˆ
ûÝ@+«	X™I¿¾¶x¢~¶¿ç
>¢¨!¿Ü'|ÉV¿Ü^-ØÖ¿á(aNcæ¿×	ýDcÝAGNbll3FGL J1219.7-03141RXS J121946.0-031419?ïþvxµÑç?±ËðáHm?(˜vBÓ?±ËðáHm?ïòÖÃE?a÷œ"ß'?ZRzfo•û?a÷œ"ß'?ïùæuaÎI?89ׁêëP?Hf+'i'?89ׁêëP?ïö2WÑ«?;7Fq|Q?S›RÕÊA?;7Fq|Q?ïý‰%¶¦x?'ZwOëRî?3¶Ñ«^^?'ZwOëRî?ï¾.xÛ«Y?•tÃ䚖?€taÆ­o®?•tÃ䚖?ïúœwU³!?Y‰£ø±¹?EŽ!µ¨Æª?Y‰£ø±¹?ï✻É*'?XŸJ>¯ÁŽ?mcCÿÛ®A?XŸJ>¯ÁŽAGN4FGL J1219.7+0444?ï¨,°sa@P˜0O‹YÀ:Ÿ܉Ù2À<rœ…dž@ 0]E«Zâ?þÚÝð,M?Ä˒ûoÍm?½håq´MO?÷ÚÀZ΂¯@—ÎxèI¿ïI$i¢?ïü¿ÙŸC'¿Ð3VćÙÔ¿ß«Ø ër¿ã¨bõ˜ñ¿Îîï¡ãê÷AGNbllNVSS J121945+044621?ïþO^7ï?Ja÷H2p?+
)ãÑf?Ja÷H2p?ïë6/øý>?eD=Kßò?dÉÐ@¼2?eD=Kßò?ïñÍO~˜a?g°"²?\ean«?g°"²?ïԇff;s?\ åÑ4?u¼Lì~®0?\ åÑ4?ïü¨d/ ÷?4Ûa¨1¸ ?:¼ÝI6d?4Ûa¨1¸ ?ï¨-Új?ˆ¤'ÉŽ?…ùô'†H'?ˆ¤'ÉŽ?ïèï˲ùð?v
m½NQ?g4mgà?v
m½NQ?ï=LÃÊg?…:¡Qùç?˜\i>?…:¡QùçAGN4FGL J1219.9+6056¿ãJÂG¸¦@KãEŒÒ
úÀ:ìdoa'À<͒…©!Í@&ðڞ@VŽà3·?»{ÚÉðO¿´á%Ž?øeLöRØ@ãƒJLÕF?í4VCÙ¿è7…½Äœ'¿ëË!{û¤¿Á›!Äuæ6¿ß؜cÎ[˜¿ïÿõEq#AGNbcu3FGL J1220.3+605587GB 121716.0+611442?ïþc+ã!'?!°¬æqN*?)ÍB5AŠ8?!°¬æqN*?ïõÉë=rŸ?U	ȤÅ?Tl)H¡£	?U	ȤÅ?ïèßÿsVÿ?n²`œANˆ?g J°Ø?n²`œANˆ?ïöy"¡'?9ΡI‰?SØ,³±ƒ?9ΡI‰?ïø·ê<ŸC?Q~G‹áFk?M V˜öœp?Q~G‹áFk?ïÛKH[l?sßÓ1ç=ò?rZ[ÒIõ~?sßÓ1ç=ò?ï¾°£æˆ?ƒâIc.Ï%?€S×A¯õ?ƒâIc.Ï%?ïÁãâÁ?oÁ—-'ZF?~š{?oÁ—-'ZFAGN4FGL J1220.1+7105?äÉ#tú(@Fèdìé¢ÆÀ8¨Ê^]ƒiÀ;ñY¡\º@R'Ž7»@'a|ÚQ?£9hs³?ÀÃøzût@­'w>$ÿ@ Ú¨Ø{Ø¿Ìe{Yè~¯¿ß?YÐ,¿ãÒú
w·È¿ælfû·›ã¿éÍ•I¨À¿ê7@Iq8AGNfsrq3FGL J1220.2+7105S5 1217+71?ïø͚ŽGg?Pj³@Ir@?LɕO	ˆ?Pj³@Ir@?ïí'Ÿšÿ9?u¢ª¾i?bØ`ûÆ£?u¢ª¾i?ﮊÐå‰?ˆÓý*©?"]KÉ ×¦?ˆÓý*©?ïýâ3¼E?+Éܬ—kª?7 ï34?+Éܬ—kª?ïÝ(—Â?tÔ¾@––?qkù–6??tÔ¾@––?ïÊ÷F?†`rýÅ!?zþrü<Í?†`rýÅ!?ïZÄㅇ$?"š¶è‰?"§c'¾·u?"š¶è‰?ïôI/Žì?K߆ø¥?Wmɱ`Fÿ?K߆ø¥AGN4FGL J1220.1+3432?ï=™Ï'"·@T»ìª¸¦À9áéÃ}˜²À<pȖg"@°˜a¶(q@l÷¢cl·?´زP\?®¼œVÉw?ù³·‡Á*@	·nN<N?ï"ÊÀ9¿Ü…SÜ¡@¿âÓŠS«¿á¤…†"¿å>þ]hã¿á,1·20ÕAGNbll3FGL J1220.2+3434GB2 1217+348?ïþ]°´î?VÒÄ@:¥?*$úJ8,$?VÒÄ@:¥?ïôØ7A¾D?X8äæZ¥±?VO'a˜/?X8äæZ¥±?ï÷5x:?U:;tÿ?Q•ÈgK?U:;tÿ?ïÙdü²C?\aI¸›û?sMóG¦V?\aI¸›û?ïüø±'Ÿ?/>ñû­ýS?8:ue‰¾?/>ñû­ýS?ïډÆ4N´?yé?Ÿ×9 ?r»ÞùnB?yé?Ÿ×9 ?ïò™Øƒº4?k9ø¦Ìè?ZÌO*÷4?k9ø¦Ìè?ïÿøPç­?w\#ò†R?‹ÀöèÇ?w\#ò†RAGN4FGL J1220.2-3713?æüA±"Ç@9;·Ç'
1À:?ÐW›ÈHÀ<`«l)ôÆ@ ã(å?þT·Æ«K?ÀÖ3hb??¼,žïnã8?ý©ÙgåÂg?ûkcˆ»zë?ïûG¿1X¾¿àœÊr/ȿޔÒ?R{M¿Þ@)È¿ÜjÈéÕF¿è]'ømåAGNbcu3FGL J1220.1-37152MASS J12201982-3714137?ïûx»lkþ?6þ8+@÷?B –ý?6þ8+@÷?ïºÕ˜<;3?"ø'Ådw?J™öp"?"ø'Ådw?ïìöþ¤‹:?cûXœhr?c	ƒP=˜?cûXœhr?ïd'k÷o?s‡_ÅäV{?"{‡üj?s‡_ÅäV{?ïò2IÔ4u?Q0Mä.$@?[›lª
µ>?Q0Mä.$@?î‰l™[[?³>+ôo?§nÉ2ú®P?³>+ôo?ïÞ.õòò?tÔ󺵑?pè"úØN7?tÔ󺵑?ì×õqýk?Ÿ,¨H—?¹@W
¹ï(?Ÿ,¨H—AGN4FGL J1221.3+3010¿ß'äëôÓ@T¯ke©¨À7ڊèü®<À;/jWWÖ@ Ó]<F,?ú£%"R? B³·[? ³~µßî@ƒy³J@a· D%¿âSÇÝúœ"¿Æ‹sü|ô¿ÜÁ¿àáW¿Ñ†±_ˆý¿Ý—|ˆçš®¿Ã[Â"¹=AGNbll3FGL J1221.3+3010PG 1218+304?ïþžÙŸn?¸Ç´*?&iÝâ¢?¸Ç´*?ïõçìÉþw?W"åX8?T0&•>`Ñ?W"åX8?ï¡I˜¶?Š¶#U). ?‡¹-¤!3·?Š¶#U). ?ïì­z¢§?WÉӌô3ˆ?cR…sõØ£?WÉӌô3ˆ?ïüß×
ÿ?3üë[?9Fåi?3üë[?ïÛ¦;µÛ?v,ؼÌNû?rs,êd"l?v,ؼÌNû?ï‰#Âkº?ÕåV.Öo?º·DI?ÕåV.Öo?ïÞA_=J?jöõXÉÓ?pü_Wð?jöõXÉÓAGN4FGL J1221.5+2814?éС@Š'H@TÒ//˜tÀ8%\±À;¶i©çÅw@ò®¸dµâ@A(¿<?—`°Þžu:?•š'Ç!?ú/<-­¸@çuXǗY¿Ý—m$E¯¿à¼J~Sm¿ãGüMÃØ2¿àvÚ݆®Z¿æþ\'ÑN¿â°–5a
ÝAGNbll3FGL J1221.4+2814W Comae?ïþÞŽe?66è8.Á?"žîœ2?66è8.Á?ï÷J×÷Î?U!/´yŸ?QkÇ×$M?U!/´yŸ?ïãëk0™?zwĊƆy?l"|nN‰?zwĊƆy?ïþó:Ÿ¹?mßh–ÞÅ? ÌR
H¥œ?mßh–ÞÅ?ïþ8Ý?$ë7U0¦?,~s'ˆê?$ë7U0¦?ïÙT5í?}ƒD§6'?sUåA½)Œ?}ƒD§6'?ïÜú%q?€'æ¹ÀP?qÀÆ[R?€'æ¹ÀP?ïÿÓ¨o\?çØ囲?¥Žå¡ˆ
?çØ囲AGN4FGL J1222.0-4121¿Â¹¤"ŒË@5+ç:6\³À;R[LVñÀ<žË'±ñ@Û®Š—s$?þ鬆Ü'´?ع¶…Ä´?Ó¾-b8Ú<?ùÕt;;?@äïp¶Ç¿íjΪó^?îž8£NN¿â/0¤ãy·¿Ùzˆ|Ê=¿ìNOÿFǐ¿ïÃn_E°AGNbcuPKS 1219-411?ïéwêa!?`Ÿ"‹.¸ ?fˆ¤^D?`Ÿ"‹.¸ ?ïÛ Å\ëé?uRZàÒ?r/_øgH?uRZàÒ?ïSWÇMm,?…pD¬²R?••*ð{?…pD¬²R?ïØm˛°†?W_µcvâR?sÉ&yå?W_µcvâR?ïÞµg!ï‹?kæ÷j-é?p¥Ld¹f^?kæ÷j-é?ï\k‹iU.? R and?"rŽŠ>TF? R and?îžfÕC‹=?™ý¬·°:?¦'®[4?™ý¬·°:?ïF™Äu?…ÅãK)Ï%?—.ÂVf?…ÅãK)Ï%AGN4FGL J1222.5+0414¿áL²P¨A±@P…à`þG™À8©åÂg=À;ÁR4€:M@`5C-Ò @{íx:¤?ª	*\[0ä?¸ªê¤ÏÛ@¥åNë @R'{ÅÉ"¿Ù€	e.'õ¿å‰>7s3Ô¿ê$úö«Ãh¿ë©%þ—J¿î]¦Ùóü¼¿ïô[¼¿8AGNfsrq3FGL J1222.4+04144C +04.42?ïý²É҂ª?'¿}¡*–?2i±è,
?'¿}¡*–?ïò÷]¼k"?e·cõkÿ?ZDÔ û7?e·cõkÿ?ïËo«CÓ?w²	ò"Õ?zH*l_V¬?w²	ò"Õ?ïúTÀ?.?98QÕ[£×?F¬ýÀ~Ì?98QÕ[£×?ïü·?`¬Ø?>'"è¸Ç^?:F4"«?>'"è¸Ç^?ïÅlcß4?Œ?ސ×?}IÎæ%?Œ?ސ×?諒X²ëò?…UZC{&}?†©Ö´Ÿ]?…UZC{&}?ïéucü¡?]$–¸•¿?fŠ›âb¢ð?]$–¸•¿AGN4FGL J1223.0+1100¿ì8W«žºý@R#ƒQX¸(À:èâ©­ãÓÀ<'Üo×ÿ0@çQÛiô?ü¢\¶º<?ϲ'´¤ã?̯ÀâÞ±ý?þæ"/•ð@8Ca©"7¿íœºëù¸¾?¯Þcß3½Ù¿çÖåŠ2ôI¿ÂÀbX¯o¿â¡¬ÃB	¿í"M!ÆÏ2AGNbcuSDSS J122307.24+110038.2?ïý©ÛÜ	?&hAm|L—?3z¯	©e?&hAm|L—?ïïÙNë?`™göV"?`o&‹}t¼?`™göV"?ïåÒÞQ?^&s:îì?j-â±b±?^&s:îì?ïëC·S­–?KAñØJè7?d¼Hށç?KAñØJè7?ïý³IŠÚ?(¶é‡é`˜?2e·Á;Êo?(¶é‡é`˜?﹕ùÛ×?‹}zYVkC?šœ13?‹}zYVkC?ïÕøƒp°?w8?ú#l¡?u¾R?û´?w8?ú#l¡?ï"{Á±)?yÜ,´é)?Šá¡t¯?yÜ,´é)AGN4FGL J1223.3+1213?Òçs刎@Rm®ˆ*ÜÀ:Ü<I\jdÀ<d É8Ö@ãw¾RŒ@é§;BÌ-?Í]f"â?¸†›:…?à±¢z¾¸@ámÛhò¿È–œd$AÔ¿å"«=0¿êî±##·¿ÕO*u¿ï¦Òœðf/?íI'w"AGNbll3FGL J1223.2+1215MG1 J122332+1208?ïúxqÏ{?BÆè'•#Õ?Fò–7rß?BÆè'•#Õ?ïò%T€éR?csKq
?[µW[¢»F?csKq
?ïÏ÷>Ý?qLcæn[k?xxô6¡?qLcæn[k?ïõâÙI¤?APJð«rÿ?T:N/åØ+?APJð«rÿ?ïø}GÜì?K*=ºübã?N
ààl¸'?K*=ºübã?ï»;ÈX?'ˆÓå¤?=1Pro?'ˆÓå¤?ïÏÏa=Þ?|·œ›K?x}o­e?|·œ›K?ï¢vÍð@ù?{ìaW}Ô8?‡bLƒïÁÍ?{ìaW}Ô8AGN4FGL J1223.5+0818?í
ÍÈd!,@Qƒ±mÀ:Å@ªÀ3À<Šéåˆ@ ׬NÓ?ý–:iˆYÖ?ÃЎã³F?·¨˜:	?õÕêî ¬@	nÀ
òwV¿ïû5•äs?ïÿ¢bô¿Ù·?œÎ€¿Û@G¿é=A^Å\?"ÄÃhõãAGNbll3FGL J1223.3+0818SDSS J122327.49+082030.4?ïþ¼¸FqÃ?xNør"ê?$4{:Tô??xNør"ê?ïôֈ&Cz?XeB_+È?VRð1êªw?XeB_+È?ïÞ-ǰЏ?p+çSû?pé&çÌ^?p+çSû?ï÷m8¬]°?<ó&huu?Q%ŽµQ?<ó&huu?ïüð ³á'?2F¤6qG‹?8zúë}R}?2F¤6qG‹?ïÈÏsO?ƒâ?ƒß¯?{˜|üf€°?ƒâ?ƒß¯?﹦ñ,8Ô?…J¹DO¦?–C³9üò?…J¹DO¦?ïäi£ª#?_'ùìØíU?k–\O¤È?_'ùìØíUAGN4FGL J1223.6-3032?êä¸oóƒ@?ò'B³÷À:Ìsí7¦_À<~ã¬bå@!âv"° š?ù"»¶úÓp?РS\žfˆ?¶çxŸ£ô¼?áqºøŽòw?üHÈK2ÙF?ïýœ"Šï]¿á¹ddIV¿í½÷|£¿?á[æ°£¡Z¿à-ä>ÙZ¿Ñ"î¬ñe3AGNbll3FGL J1223.3-3028NVSS J122337-303246?ïþ4ÃE?. 
˜sž?/¼°Û"âª?. 
˜sž?ïœ=Á?bðÁ·°†÷?anQ2GÞå?bðÁ·°†÷?ïØ>µ>Þ?y
$ë͑?sûà—¢!?y
$ë͑?ï:q?JY™sããN?`sO"7?JY™sããN?ïýtCÖ?4#Ž¢ûrŒ?4]ç}>?4#Ž¢ûrŒ?ï½ÇI2×v?"¯è–†?€Ž-¬Âàu?"¯è–†?ïÌ[ò*e•?€¸à±&ˆ?yÒâŽ%U?€¸à±&ˆ?ïÂCÁ>Ø?skø?M
?~Þp¢Ð0!?skø?M
AGN4FGL J1223.8+4649¿¾'åÚhœ@Qda¦
EcÀ;ŠRuÚÀ<í±jp·"@QP=/5x@Ç¢ PØ`?É|üÕÔ¿Õ>bŠ?³ÝÝ@bp¸@°"õ¦o?ÝCiv¼¿ç'Õ1\½¿ã§gž¿â1_œÈù¿âdµ—&¿ïýAt>–>AGNbllRX J1223.8+4651?ïýmËNaQ?&‡çø)]?4'¦˜Ìd?&‡çø)]?ï÷éq¯V?O÷îö?P-†ª<?O÷îö?ïô#p7î?U©˜L_ýˆ?W¸å	'¤€?U©˜L_ýˆ?ïöúu|ƒß?5""|jž ?R@±±u?5""|jž ?ïüÔ¸IÏ?0àя8d?9Z@Tîös?0àя8d?ïߑ/½²Ó?s;|£ÙªQ?p7h.å/?s;|£ÙªQ?ïóE_¹+¹?gzV±ˆ:Ü?Yu@¹£Ž1?gzV±ˆ:Ü?ïØ{–›¯Á?aoöž\•æ?sÂ4œ*Ÿ¼?aoöž\•æAGN4FGL J1223.8+8039?̅ø…•ß.@B2u¸eÀ9dFøâÕÀ<®=•ŒÅ@^.$*¬§@ð[|þX`?¯¤b ^.ß?ÀE™'7Ð@11eәp@
<Èý	€‡¿Ýe[#'+f¿Ý)Ucߣi¿ã£C_1¿âøû^°¿è9îlȿ캫ݓïaAGNbll3FGL J1222.7+8041S5 1221+80?ïùü%*?Bê™;F'?HjrƒT?Bê™;F'?ï¾ï¿kn?‡[ðŠü?€D!œ¤?‡[ðŠü?ïÙ÷Ķí?qߑz°-+?s°7ëR?qߑz°-+?ïX¥{­¨ù?s"êéÞx?"ëP†ÛDí?s"êéÞx?ï|¨E•Â?"úþ˜´²É?j÷H5Ð?"úþ˜´²É?ît‡¼Lw?°÷"÷sj?§(·‡ªÔ‹?°÷"÷sj?îÒÌ]¼Ó?š}ï͋l8?¢Ó:òŸÖ?š}ï͋l8?ëSÎ8²¤?¤31GÛÝ?°Ç5où?¤31GÛÝAGN4FGL J1223.9+7954?Õ˳HRW@B''͖ À;Q,50"À<ãQN§-@!Ç&Š-jò?úâ_:øúR?Ζ[K«$?Â58†">?ñÇ7a–@Qõx'â?ïÊýê¦ý¿ëÒ§7E¿Ó"MA§?J¿Ø݂'™¿¹T÷S3-Õ¿éh¿§J\EAGNbll3FGL J1222.7+7952NVSS J122358+795329?ïþØ.™ŠD?eÕî?"}v5îõ?eÕî?ïõ¶}!‹7?V+WauB?T"A7¡»?V+WauB?ïõ±•cÔç?U	Ò¥øwH?TœÕr¢l?U	Ò¥øwH?ïödí"A2?:G­)ÐÝ?S6$ց]	?:G­)ÐÝ?ïþLŸr»?%áςz"T?+>ˆøå-?%áςz"T?ïÔCVÊo®?uO×-ÎÅJ?uÞT‡Ù?uO×-ÎÅJ?ïóY¿ö
ð?dì~ q]'?YL€H$0?dì~ q]'?ïàmþW«°?aµ­ÅWR?o'¦ôx?aµ­ÅWRAGN4FGL J1223.9+5000¿à€«6­™´@P¡]N°À9¯£¯À<:ʄóð'@³ªºG@YÀª›?³3Áù_'?ÌÁ³éüÞb@-nÎõ@þû¡v‡Ç¿Ì^ÕùFRu¿à4øÀEªÚ¿ç܃ÄE>οèçüÓû•7¿ìÙ@¿ïÿß´0ÕAGNfsrq3FGL J1224.5+4957SBS 1221+503?零C+W?}[loba?†So<¢?}[loba?ïï'&*-?cwôòyH?`mÙÆ´«?cwôòyH?ï•€å?"tqÇ¥?Ÿ-_q›ü?"tqÇ¥?ïçüì­ÆU?QšS«1GO?h/ݓD?QšS«1GO?ï~"ÌP%1?‡1¼»3ó?-†o!Ý?‡1¼»3ó?ïÆT¸
•R?'Jˆ³?|Õ¤
ó'?'Jˆ³?í¦ò^Æxº?¢Úå1{*Ì?²Èm"1?¢Úå1{*Ì?ïSºôvù ?€ÞÜ7"–Ê?•ˆ¡kùaü?€ÞÜ7"–ÊAGN4FGL J1224.1+2239¿äiÛȚõ@T—W'ŽžÀ;^ÆùN5À<¨§<‹Â@"p~]?ÿßCÇÕí?½Ð­¬ö¿"ãL@€?ýáçÌ,"Ý?ý%.»TTk?ë˜> N¿¿íA+®Ús~¿árߪJ¿æž©/"¿ÂúŒ¤¿ÙƒöduË^AGNbllTXS 1221+229?ïývg)H½?%±ô~QOj?4LƲ?%±ô~QOj?ïŸÅ±ê70?›4Ìõ¨?ˆ"{#`"?›4Ìõ¨?ïéXˆ0Í?gE&ߤ?f§x*?gE&ߤ?ïת'Âg?dÓÀÙdåÒ?t*·öÌa?dÓÀÙdåÒ?ïø^€¾×A?HòíEa"'?N…ýð{^Û?HòíEa"'?îCTq­}?ºÆC6Ð;?«Ê¸å('*?ºÆC6Ð;?ï×َãCm?{ß:±®m¤?t8•=z?{ß:±®m¤?í¶'id?¬ÜªÆ»(?²KïlFë›?¬ÜªÆ»(AGN4FGL J1224.4+2436?»­ÐS¹@TÛÀ~à°¯À8ûDæ¹ÝÝÀ;æàyQûu@А'‰Úà?ýג"¬Ó2?¨³×]tzP?©²Ð]Œ3f@ç|¯Ý©@¾wä"?ª¡;¾5ôó?±qÚbâx[¿Þw†®‹¿ÜKêd7b¿ãŸ¥'(^¿ÐjiÀ¸íGAGNbll3FGL J1224.5+2436MS 1221.8+2452?ïþÿ8s¨³?¿ë8r? u !?¿ë8r?ï÷œ8|À'?R¯Ôö:O?Pǎ¦IËé?R¯Ôö:O?ïóãR'ó˜?c—9èc+?X9[ÈÖ©?c—9èc+?ïþ~õmC¿?'Ù8î?(«§H˜¥?'Ù8î?ïþíI«*ø?£X2u•?!+e²x7=?£X2u•?ï×X©ºN?z¦C+9óÎ?tS«CÕ2È?z¦C+9óÎ?ïö5zÇX?an#ªñÝ?Sù•ˆâïþ?an#ªñÝ?ïþ!Òsæé?%Os5¨O?-âًàÙn?%Os5¨OAGN4FGL J1224.7-8313?ì
•k9×À4e¿œb¡¶À9lʍWkøÀ;ü¢¥±ÕÑ@®¶â)Ö@Ø©_	zÓ?²¦_¿r
"?³¾õsµ'?ývqüœž1@
!+˜	K®?§]	pl#À¿æjW®Î¿çèGçöÿ¿éILÌKž¿åÓ´EíJ¿ïÿË&Ú_]AGNbcu3FGL J1224.6-8312PKS 1221-82?ïþ=ÍbkQ?/Qq£Ì)?,#)ƒ‡Û¹?/Qq£Ì)?ïòx'óÚ?]3µ²Q?[ú"?]3µ²Q?ïí²&?[íU˜ '?bMÙ–S?[íU˜ '?ïñRqî?Fl3yÕ±?][Ñ¢ "•?Fl3yÕ±?ïþ‡éT(2?"V4aƃ?'j7Xôý?"V4aƃ?ïØV-&æ?v·0S'ù?sÔýIDë?v·0S'ù?ïÜÉ
0Á¥?rrQfZ%?q›zõ]g?rrQfZ%?ï ~³—Ð?w˜M€¤ž?‡àSœ\i?w˜M€¤žAGN4FGL J1224.9+2122¿ênÍEn@TjWÑx-8À6Y‹zՉÀ:üÎqèz¨@ã™%ÖS^@9{úLaØ?'<cï¤Ï>?§|€Úš@aS¢>ƒÉ@#؅c¬¢¶¿Ð[¬Cjbõ¿â{R¼ev|¿å¤«{Cm=¿å³@ߙ-¿çÒ(@æпäâÀ‰Èk>AGNFSRQ3FGL J1224.9+21224C +21.35?ï÷÷ŽJ
É?Mš–CS?P㻡3?Mš–CS?ïò­å‰¿?d,sŒ%?Z¤4¢¨ò·?d,sŒ%?ïÊð`ªÇ?¨tPƒ?z‡ÐøЩ?¨tPƒ?ïÿîä5€>â×NIŽ# >áëg؍ž>â×NIŽ# ?ïøîf$¢!?E™3ð¬Ï?LFhr™ËO?E™3ð¬Ï?ïË?ØÌÏ?ƒ²ì…0¢P?z`éɛ?ƒ²ì…0¢P?ïÓéÜ.?'×X¦ûÌ?vsOº?'×X¦ûÌ?ïÿêc%A>ík$¼ÿ>圹~
sŒ>ík$¼ÿAGN4FGL J1224.9+4334?àzµÊ	h@R-gôÛߏÀ9çÁŸr ¯À<•ª¨µ–O@zýÕÙ:ï@kh¢×0?±ãˆP m?–œÇ nM?âF$!Gxe@ÁçAî
¿Ò1žBuÆ¿ä,4 ˜ü¼¿æ§‡-†K¿âÚ|îh(¿ë1Ûz¹×¿ïÿúŒ—ÓAGNbll3FGL J1224.6+4332B3 1222+438?ïçE"¢N?b/ØiqáT?hº{yc'M?b/ØiqáT?ïèÓÏ($j?rڌ3µ?g,1t=±?rڌ3µ?ïK—Ûî)?ËgJ{Ÿ?–"k4à?ËgJ{Ÿ?ïaV˜×ÁŒ?ƒˆ'uG§?"Õ,ãPz?ƒˆ'uG§?vÅP¤?ƒ_̲¸[÷?ŠP"U‹÷?ƒ_̲¸[÷?ïÁ9ÂT´ô?ƒ/RæÈDª?cäÃÍÃ?ƒ/RæÈDª?îüJê<§Ú?–´×›Yxœ? ;Q_¥`?–´×›Yxœ?í+¨ÂMå3?©¤8U?¶¢¹ïH¤i?©¤8UAGN4FGL J1225.0+0330¿âüj´©ÀX@PcJ¡!À:Fþ»\bÀ;º2ƒàʱ@{õ&]6è@-{~%ŸÍ?Å>éõ§Œv?Ö,Ôz¿d@Q)`Kš2@×ͧS¿ÒÏß[š°p¿àìJ«õ¼°¿ßªT|ÙðL¿ê eêV ¿ë68Ág"ã¿ïûµ¸´AGNfsrq4C +03.23?ïßƘ;†Ð?jÏdƒÄv?p³Þ	?jÏdƒÄv?ïô/9þš?[ƒzr[Âì?W¡Þ?Zó?[ƒzr[Âì?íùXþžñ?œÃ÷b¸áý?°5?o/!|?œÃ÷b¸áý?ïþ¥É—|ù?ÝGŒÖˆî?%£g"¶*?ÝGŒÖˆî?ïÃ$Òè?µ3®DU?~mö'
G?µ3®DU?ïdžA֗¯?€ÄJˆ"''?|<ß.!D)?€ÄJˆ"''?ëÝ©ÈZ€?¨AÌyÑäJ?À‰[üޖ?¨AÌyÑäJ?ïúGâAÔ?=ó¾²ß²A?Fàvh¦›È?=ó¾²ß²AAGN4FGL J1225.3-3446¿'Éßίj"@;Èä†&öÀ;;ª]6;üÀ<›ÅPä@ e;Ó÷Ž@òü¬Žhä?¸xƒÚ¿¬-£ <G?ìnƒÖ¹µ™?þ¨XÓÖ¬¿áo0«¼²¿åT[זT¿éjêŸpž#¿Öö†oj¿ÒfuÞÝq¿Ý""ܯAGNbcu3FGL J1225.4-34481RXS J122534.0-344737?ïý ‡ètÒ?*àHç܍?6ûÀû†&?*àHç܍?ï~Æ?_XT²¹@?`kqi*
H?_XT²¹@?ïò¯	˜Z)?HmÝTFGV?Z¡ì'ҍ|?HmÝTFGV?ïúÏj?0ˆ¡•'?DÂTö+K:?0ˆ¡•'?ï÷ŠYÏn?M5÷5Ø?PëLåýø?M5÷5Ø?ﮩ<·Á?‰"yŠŠ¦ð?"U¹íºi±?‰"yŠŠ¦ð?ïòGœ2|?cÙ¾!ä+c?[pÇèàG_?cÙ¾!ä+c?ïő¬\·2?r™Úq"—?}7)ñ@Ε?r™Úq"—AGN4FGL J1225.4-1550?·ÿïˆëIÛ@GHf^ê–À;Á_0ϬÀ<ÔL~]Óñ@"8u¹•?óv ž9%?æT~!nÑ?á–
˜à66?ÿw¤as¸_@—|Hzî¿î¹6b<¶?íkawê?ΞŠŒ‹i?íêó((Š¿Ä õÙ`ƒù¿æåfâOAGNbcu1RXS J122525.2-155251?ïìU;Þ(?¢-4þf?cªÄŅpn?¢-4þf?ïñÕ5ã"
?c·ä½?\U"Ryå?c·ä½?ïº4‹;̤?wZâ\Րº?rÝ+åm?wZâ\Րº?ïúN뒋?=jš°:Å?FÇ÷Ò·y?=jš°:Å?ïù¸ò¿•?LFãä6ÖY?I5}vá?LFãä6ÖY?ï½J¢ªS??"¥`ªÃ@:?€­WTcN@?"¥`ªÃ@:?ïºùÄ/Lý?†n§?¹?AŽøLH«?†n§?¹?ïóîlYÅn?W–ãs7É0?X#&ÙD9?W–ãs7É0AGN4FGL J1225.5-2851?åðæÅFp¨@@Õc¡ À:……žÙÀ<\>ª_º{@¾DVñÿ6@¢ÃÉîËû?ÎRÚ'C?ÕX"Ì@Ž-À,«Z@	OS;;jd?ï¨3PD¼¿ÚYÞb÷F¿âQ žÛøº¿ì˜Á‹¦¿ÙàÀI±¥¿ïüvÄ AGNbcuAT20G J122515-284956?ïøIä`Î]?M›ëX#d?NØnQ+Ò?M›ëX#d?ïïÄiY"x?aÏa—±†?`;–zqˆs?aÏa—±†?ï~^¤Èn;?…êèÿxê¤?4+jaÔ¤?…êèÿxê¤?ïñ>Õ‰
?CàCìª?]'VU"ül?CàCìª?ïóu¼³Ð?[·%8,ò?YÀ†˜`	?[·%8,ò?ï½`¡ç'?€¸"óT]ì?€§×"-þn?€¸"óT]ì?îþ"ᒒÐ?–§žõ6? Ñç²¹ù?–§žõ6?ï±Ü9.þN?sÁwýQ?ƒˆñÅ's?sÁwýQAGN4FGL J1225.6-7313?ëHÅçÀ$é³ÃçÀ:0þæ$À<&A
çI@jђ"Q‰@0;7äs?½ÊÔÏû€i?§:{Ñ݂Ó?ïô&­é³@	JÊ©†ø?ïý•ø$il¿ÅÊEÞÜnÖ¿èÒ»YS¿×ª½®KØF¿äç¼Àæ¿ÜÞùÀJÞKAGNbcu3FGL J1225.7-7314PMN J1225-7313?ïþŸ…kå+?çäûÄá"?&©"ãüØ?çäûÄá"?ïò‡-Ӛ>?bŒ÷âá?Zñ¤E´y?bŒ÷âá?ïöæB¥Ó?SŠ·K¬¶ã?SÜ3ÿêO?SŠ·K¬¶ã?ïùL\2?1i:]—?JΎÁŸ´þ?1i:]—?ïþÌB}ñ?kÒ@U|?#;ԦĄñ?kÒ@U|?ïÈ»á&²?Š1¾÷žë?{¢}
\âí?Š1¾÷žë?ïñ‹	??fÔ[Òè?\àê-P®?fÔ[Òè?ïçm>"1È?VJOòÃÙ?h'Áum×?VJOòÃÙAGN4FGL J1226.0+5622¿Ô²1°Òj@N4oÞµ,À;ªß<;À<ÉLÙÍfP@ÿñº—ëï@k¯–[ ¸?Åta¼2 ¼?iDúIÚ@JæýÐ?îÐó7š¡¿èá
¡~¿åáOp€›œ¿ãâ*⬲ü¿äÁt‹Z¿ïÑqÛÖUAGNbllSDSS J122602.81+562254.6?ïþâA0Õi?'pÐÕ×?!ÛìÍGQx?'pÐÕ×?ïøS¸—i?QÐü¥‡¾?O±"H-w?QÐü¥‡¾?ïô1r5I?U@n8!™€?WüW¿?U@n8!™€?ï÷~¦¿?7G©âñ¿ç?Q³™äô?7G©âñ¿ç?ïÿ(ÍÝ? QI±,?L^MŠd? QI±,?ïÜ\©Æ"×?up'üò9?qÑ«ÍX·?up'üò9?ïðŠ!Š?h=û¢
L?^ë½5ÿŽ?h=û¢
L?ïÛð?,?a‡9"­è?rvˆ$•ß?a‡9"­èAGN4FGL J1226.7+0637¿ïúXã4Üð@Q+OKD¢À:ƎyªæÉÀ<-†K<@!? &¼x?ùUɯáÚ?ÈG•*tÝ?Â[–ÿ‹eú?ý@|&©@Ç`QN|¿ïÿÿ&¦³?ïÿýç!é¿á3ÅP˜¿Ábº_aåM¿ÙVE'¿áYgŸ÷V¹AGNbll3FGL J1226.8+06381RXS J122645.2+063906?ïÿGŒ—¹¬?
Îä0M?rúœ®?
Îä0M?ïòÏ5»V`?b£s¤?Za"oÆ?b£s¤?ïۘ®¦àÄ?z{l¸ë?r3¨ÊAø?z{l¸ë?ïøÓ¶ÿc«?6!fÕý'»?L±$WØm?6!fÕý'»?ïþ•:u'õ?"r,Ô}Ë?&¬T†ÀP?"r,Ô}Ë?ïÈdÊ*—?'sKçní?{Íý0è4B?'sKçní?ïÔZÂ:Ì?)ËÕ§Îþ?uҞڶn`?)ËÕ§Îþ?ïè×Í[èß?Z‡	ɧ?g(2šx9?Z‡	ɧAGN4FGL J1226.8-1329?´²}zÿÄ@Hxª*sÀ9‹}¼ÄÀ<¦†çæ.@LÒ*?þò]€
×?¸[ìÿŒ™?¾#әŎ@PŸ}i[@Š Õ¸"¿×y çÁÆ¿è7k§^¿ÈI?9%æo¿á€`"•¿ä¤&Eüd¿Ð7œ'"mAGNbll3FGL J1226.9-1329PMN J1226-1328?ïþ¦@Æï"?•¦Hßéñ?%›ñ/åªâ?•¦Hßéñ?ïòNPÁ?[¡x$Ñ?[céf¼ô§?[¡x$Ñ?ïòƒ
"Œ?h^Y·fò?ZùêìåGu?h^Y·fò?ïö'Á«R÷?>%'߃‰¾?RÜ|±™" ?>%'߃‰¾?ïüÂ3ç?9šÞ\}/??ñïÛí?9šÞ\}/?ïÂ+ÿ7X1?…éKñ`¤?~êS%Û¡?…éKñ`¤?ïâöCóR?y'%P¢Qõ?m	ð̊Ín?y'%P¢Qõ?ïãš[áR@?[½tî&'I?le¤U§Ë?[½tî&'IAGN4FGL J1227.1-4437¿ïð–PÂm×@2­}|,¡À;,‰ËÆ=À<šé+¨$w@!8 ¦n?üËyæuë?Ìc¶ˆ½©C?¶dt^Kº¿?흨;ic@ºì*
?Ÿ¿å­4¡Gbë?ï©3g#{¿êŒ5-w?Ö©aãŸÍ¿ãÈÊœ£¿¿r¬šÓ+AGNbllPKS 1224-443?ïÿ"ba¸Æ?)vÃ%̯?'m†+KI?)vÃ%̯?ïïÐ¥ýޛ?bgJ݋ñA?`/YãäÔö?bgJ݋ñA?ïó¸«F"
?O³'HmΜ?XŽ©Á—?O³'HmΜ?ïý£IEÄ/? t¢e¸l?2å³ú-À®? t¢e¸l?ïÿZW~/õ?«ãAvB?µŽ-–_?«ãAvB?=Œ}|?–	\7Gñ¯?ˆ–ð§/tÜ?–	\7Gñ¯?ïî¦}­«?nzÅ?aüY…4?nzÅ?ï÷ݒuk›?F>å­	5?PDÚԐ#C?F>å­	5AGN4FGL J1228.3+7521?æǧä,‡?@DØ	þ†ƒ<À;XèQ'NÀ<ý
)N­ã@<…—Y"†@è1AÁkp?ÑPÂœÇÌ?®Ùx_jÒ9?×w*#?P?ÿÀwÜÛb½?ïò…ÞѲ¿äʬ+l•U¿ÏõUҚl¿ås`'¿æ÷œ"/¥	¿¾[WáAGNbcuWN B1225.8+7537?ïý.ÿì›?-Ž?oíÔ?61ā_?-Ž?oíÔ?ïôaâu?U :ÂzŒ¯?W=î;÷å?U :ÂzŒ¯?ïâÆß"ô?rÃ*·æ˜?m9 ë¯|_?rÃ*·æ˜?ïÖ_<ü_·?UçIäDI›?tÐa—ͤ'?UçIäDI›?ïüBÂXÌ?7fŸ§ë¸ì?=éë(i66?7fŸ§ë¸ì?ïÓפÈ?uL–Dô%?vp"#¨c?uL–Dô%?ïÒ¦òâO?~ûd|6ËY?v¬†t»v3?~ûd|6ËY?ï`"a­UI?{XiÊ[E?"í"Ñ4ŽÉ?{XiÊ[EAGN4FGL J1228.7+4858?å;u 	@PíTK±¯:À9òÈlüÀ<PhÍK@áîÇôK@xéö©??»vapD?ÁA;ß,@ª#9Àëî@Þ<)Ñàˆ?ﲋ£6ÑM¿æ|zo1ç¿æÕ*Ÿû ¿ì%yÁâãå¿Ýì%!øxL¿ïÿjÿR[AGNfsrq3FGL J1228.7+4857TXS 1226+492?ïþÌY'öñ?—á7¯?#:jB_âf?—á7¯?ï÷ …±…I?P—yìwÜ?Q¾ô†÷îË?P—yìwÜ?ïã
4ûùû?pß¾U^€è?lõÊè‰%_?pß¾U^€è?ïù¾©¸9‡?3X¹Zšo–?IY·îë?3X¹Zšo–?ïý:µï¢?7&<:"Ç>?7V)]"ùg?7&<:"Ç>?ïâü4ïK?nâzTv!4?mäÚ.üï?nâzTv!4?ï‰9IÍ©l?ŠÔéúû¡[?±­šT?ŠÔéúû¡[?ïåŒf!¿e?[dóšx?js™œHŠ?[dóšxAGN4FGL J1228.7-0318¿î¡âV²ûQ@Mˆã£¨çÀ:`*yPMöÀ<YÊ1çٙ@ê¢îþG@¦^ÛX?Á6šÜ9Ò4?±áàZHJò?ðþ ŸGX"@}Ðãe–¿ä¬ýpÇ?îÙE¶Ãv¿ãñ6É>£¿àTÞ긿åÏó'ªhõ¿íþë}'üAGNbcu3FGL J1228.4-0317NVSS J122900-031758?ïþ;^ËS?åØo[è?,J Þ
'4?åØo[è?ïðq~aH´?^n¢}hž?_â¸èY?^n¢}hž?ïñi;ØÉ?lD
ÅÁ7ê?]û-ÚN2?lD
ÅÁ7ê?ïé³ðªD?P7©$»­œ?fùL÷$?P7©$»­œ?ïü5˜hA2?6-­HÏ ?>S=€"'Y?6-­HÏ ?︯Š'á'?•'àʕ?Ôc¿\?•'àʕ?ïòàp?gî4œÛë"?[ÿ¿úg ß?gî4œÛë"?蠟""Íþ?x¸L»,*?†ÖÞ|'?x¸L»,*AGN4FGL J1229.0+0202?ãÊk)«@PwpyåŸÀ6ä^}cØíÀ;HŽyªæÉ@賖ðÇÔ@ë5ó×ӑ?Š Îc*À?¸µmŠœü{@"›y·|°@!¸j¢Ž5¿Ø®gÜÞï¿æ#
%󯐿éêPkR^¿ê‹*k
•¿ëó[ÂHf¿ëŠ
_ÕR­AGNFSRQ3FGL J1229.1+02023C 273?ïdôŸµÎ•?¹EýÆÄéâ?"al¯'u?¹EýÆÄéâ?ïèäÍõkÒ?s†\"Ÿ^?g1⸵Ö?s†\"Ÿ^?îַԏ†?¢…¥™G³J?®B"Û ?¢…¥™G³J?ïþ…ÏbS\? ŸX"U?'£§×R? ŸX"U?ïàA¹ˆÍD?iOñý'P?o¾F†QV?iOñý'P?ïb#\6É?¨%Ë¡Á•¾?"¿›'ÁXè?¨%Ë¡Á•¾?îì1s?š{á~Ë?¡>\ïµ:?š{á~Ë?ïöÔHÓ>½?OkÑtÖ³?RWmóÎm?OkÑtÖ³AGN4FGL J1229.7-5304¿Ø0˜ŸÚ·'@#SA|¢À:lT¼ð·À<3uÇ,z@/äbÀ"…@úb>¹y3?·¥ÃH"™U?pN¦þYŒ?»breù7@	2tÔ¾2Ö¿Û¹4i"P¿Ø»b¿ã6쐷rÈ¿ãºI!²o¿Õ;à^d¿çú
­g¬¸AGNbll3FGL J1229.8-5305AT20G J122939-530332?ïþ>cp›?:mµ²?.œ匤_?:mµ²?ïêT	ö«?t""<GQv?e«öž<ž?t""<GQv?ïõÂt"6[?IZÛ­¸"?T{p⚯?IZÛ­¸"?ïþ'1«&?/ÑûA?&ߎ˜µ°Å?/ÑûA?ïû±zŸù?3Ç,\NêZ?A:Ÿ,?3Ç,\NêZ?ï:4ë<?¨Áç[æž?˜¾ÞŠ†?¨Áç[æž?ïõðëmª[?]²ì?š²?T)ìÙò?]²ì?š²?ïûÁˆå±?3póƒªú×?@ùÛ²*23?3póƒªú×AGN4FGL J1230.2+2517?îb/®•ô@U9ý6÷ãÒÀ8C-|:
À;pb·…<ë@Ë[HÐÿ7@ÝBeÖ?›±Ò vX?«Òƒšÿ 4@t/øì@ÓÐÜ{ì`¿Ì8¡1=®¿à‡ÂÀð¿áW_,¶Ap¿àãeË5óØ¿ä+4+€·K¿èjÜí¬@AGNbll3FGL J1230.3+2519ON 246?ïýÓq½Ä?1¡áZjĨ?79dP\?1¡áZjĨ?ïõPz§ø?^DÐs<?U_
ˌ»"?^DÐs<?ïèöësí?e§4m?g	¡ƒ»?e§4m?ïÿàuÿ"(>ä*ù!þø>ïŠ*¢‹U>ä*ù!þø?ïþÛÝК?%(£©àSS?.rEº'tó?%(£©àSS?ïØŠÛç?y‹Qe?sþtªÃØÈ?y‹Qe?ïîWaåP?p¼œŠÿ¿?a¨žÕý§Ó?p¼œŠÿ¿?ïÿà+_p>éđü°>ïÔ΁]¦#>éđü°AGN4FGL J1230.8+1223?ßMèKzÊ@RŸag#$ÈÀ8ÎIÚ>¥À;ân×N0@o&ëÒ Ÿ@5Ê¢P!?¤¾ÿô[K?¡íœƒ·b¶?ü84ú³@	=¿©"Ï¿Üj°¢õá¿Ø†3çüÔ¿ãBU&
±¿Þó·‡Á*¿æg;¾G"ÿ¿Ð6äΊAGNrdg3FGL J1230.9+1224M 87?ïþO¬™.B?«òì^ÓÌ?+:¥ó?«òì^ÓÌ?ïòÈ'²²«?\Òò¥×D?Zo±MØz?\Òò¥×D?ïòE7 2î?i¾ly3?[uÇÙ3?i¾ly3?ïو'¾¼œ?cP;ýh=Z?s;¶¥q%Ì?cP;ýh=Z?ïûtUY?;ãé¶÷Õ7?B.¬ª‰"?;ãé¶÷Õ7?ïÉ·£½+g?'q,I&h?{$.-ø¯?'q,I&h?ïíhÈ&±?r\>¿'?bå—ÞO=?r\>¿'?ï³ÎÆo?ƒÍ`fök?é‹Nœ(?ƒÍ`fökAGN4FGL J1230.9+3711?íw*Ðw @SÃXdE#öÀ;kGï'Ú:À<¥}I׺g@:P$/µ$@"¿Z'È?Åáe¶K1¿³J²«¹VÎ?îÓë¤ÿ(j@‡/.kÎ/¿ÑÓ%•|)¿êµ
(¯G¿îÕâ Â?މº¾ØBw¿ïÿèÅPØ¿éièÑæAGNbllWISE J123124.08+371102.2?ïùîûG'?D'DIk'^?HG¨Ü£T?D'DIk'^?ïô…LýÖý?Xî©wzc]?Võeƒ ¶ ?Xî©wzc]?ïÅ#Õ6¬?{KY-bu«?}nxâeÍ?{KY-bu«?ïõCvÕÒã?H|¥Ò¯K?UyâY"?H|¥Ò¯K?ï쁩Éùš?föžÕ0/?c~V;…Æ?föžÕ0/?ïÕ¢Ð5HG?€,yI†Ë?u.—ÊŽèf?€,yI†Ë?ïÄÑWdڏ?ƒ³³ó" ?}—TkÏH]?ƒ³³ó" ?ïŠWÊä?‰Ì¿Æ/øâ?~ê	×@Ú?‰Ì¿Æ/øâAGN4FGL J1231.5+1421?搸®ÿÿ¢@SÀY!À:YoÒòåÀ<]|Ìy1@ ©.§ˆD³?þ8RÆvq?¼é}1®ù¨¿vª­Nh?½Yۓ"@°ÊnΔÎ?ïڋ1!
<¿èŸݵR]¿ä7sŸ4
N¿Ó¢yg¿ár6é¡꿳ÆóDç›AGNbll3FGL J1231.8+1421GB6 J1231+1421?ïýâ'¾? CMފ?0ïÞ!æê? CMފ?ïô³‹ˆ3ì?bFŠEñ(Z?V˜èšaÙM?bFŠEñ(Z?ï÷8‰ðjr?c¡®)3V?QŽëùÌÉ?c¡®)3V?ïõòeì ®?=ëZÐÎ+?T4N:Dz?=ëZÐÎ+?ïýBâL'?'$Öí•?5ï¿ÅÖ´¢?'$Öí•?ïÎ1ªƒ2
?'\K…dƒb?xç*Ÿz?'\K…dƒb?ïú#Á‰²?YQõ\L©?GpûSôTË?YQõ\L©?ïã®e%0?YWœãUC?lQ›¤?û?YWœãUCAGN4FGL J1231.6+6415?åÀ"šl[@J^j¹¦À:"k†`×±À<µ+úYÍÒ@ 0@ºÛ2Á?þƒ†'e n?·8Ô²ÊB.?)˜£i—ïY@sVOiu?ß^ќ•Lƒ¿Úª¶AÅó¿ã²¡r«ï¿Óù5@S­&¿ájQýù•ƒ¿ÄÁK#êÀÔAGNbll3FGL J1231.5+6414MS 1229.2+6430?ïüFŒxÁ)?/ÜÆ2ŏ?=˜êü.<?/ÜÆ2ŏ?ïõøÃÜÊW?S"«×âe?Tx˜áñt?S"«×âe?ïï¤gÔG?fç&º-&?`[™È!'?fç&º-&?ïêR|"h?L¯k×±?eî­¾…ßm?L¯k×±?ïøvúmˆ?E›lS?N$O€øÓ?E›lS?ïÜ¢©ýXË?qØcha²?q®«!ŸîŽ?qØcha²?ïðփs¬9?l¸wiì?^Rø"¶ŽÓ?l¸wiì?ïÄr›S1?fLBDéT?}Ʋ`ϯ?fLBDéTAGN4FGL J1231.7+2847¿æ×1j0Jv@UUüã
®À8—|¼êºÀ;ÒÚý87@^ܯC?ÿFVüfŒ?¡šØÞÓàg?¤:à"BM
@	Dzãí@Û°ºG?ï÷ü@WÞä¿Þi"nå¿àWësÿߏÆ­°}¿à6YSXm¿åRÓº}AGNbll3FGL J1231.7+2847B2 1229+29?ïý†?8"ß?cW‹7B?Í?3Î!·Ä9?cW‹7B?Í?ï÷F ÝÄ?WÇD191E?Qr¿HSxœ?WÇD191E?ïíAg1?mòÈ(µJ?bá¾Ñ(}€?mòÈ(µJ?ïþT£LÃ?1+=Lv–?*¾¥":c?1+=Lv–?ïý'…†Åµ?)ÍtMõ«?3kÕÐʈ?)ÍtMõ«?ïÛýÑÉÙ?yÍÅ]?rĜ?yÍÅ]?ïàí?z²í<SÏR?oý">Cµ?z²í<SÏR?ïþAúÔЅ?"ú¡¯Ý9Â?+àRڌÊV?"ú¡¯Ý9ÂAGN4FGL J1232.5+4821?íøzá®Â@Qm3	AÈÀ:%…—"¤À<†Ó«.í@Xûu·P@_ND0±?¸½gÔûox?³^óUw«³?ø¯²$ªÚ4@m™È"'?²PúŠet¿âÜb¡µÇοãø™]3¸¿çž<á²·ù¿ÜæÿŸ¿ïÿó v,­AGNfsrqGB 1230+486?ïû^Öw?2~b #"…?B‡ö¯é½d?2~b #"…?ïòŠŒ"0?Z—GÄ_¢?ZêæzŠ@#?Z—GÄ_¢?ïìÁÞ ùy?ioÐ]Öÿ?c>!?j?ioÐ]Öÿ?ïÄچZï?c8yeëðë?}'¼ÝJÜ8?c8yeëðë?ïó¥¬Ly«?O§ä×kæ?X´§Hб?O§ä×kæ?ïÎ1ÓPŽR?y=Àu;™q?xçwU>þ?y=Àu;™q?ïÇV#ß>{?'—¢æ?|Tîp†­?'—¢æ?§T9µ?¸ŽC¨Šô?¤Æå‡LÈ­?¸ŽC¨ŠôAGN4FGL J1232.5-3720¿î<¥dþÝ@@9`ð¸,,À:'…€ÞÀ<M57ð1V@ Ӏñ5?þräùê<?·Óó?"ª—e.Ok?à3
^RÆ¡@ntÊ­7Ü?Òa¤W׿εœ¯x©¿àä/¿á,¿à)ᕱ¿ÉçΰқC¿å_iòâáAGNbcu3FGL J1232.5-3720NVSS J123235-372051?ïüҀP'?4£_çe‹?9kúÃz4?4£_çe‹?ïóÀaâü˜?\§°o¤Ì?X;í'.?\§°o¤Ì?ïóAÙǺ?h_e?Y|LfÞ?h_e?ïûjh˜^ ?)¡ \
?BV^m:Ì%?)¡ \
?ïù%(a%½?AøQŸ'Í¢?Kk]²¿Û¥?AøQŸ'Í¢?ïօDõ9?uúÿ¤MV?t½?Zų¨?uúÿ¤MV?ïï+€{)[?q­ŸJ\"?`Ô²1|å?q­ŸJ\"?ïóK¼–ô¤?J›	ß´Ÿ"?Yh†|ài?J›	ß´Ÿ"AGN4FGL J1233.1+1703¿íN¾:Ò}«@SÄÝ?á—_À:ûÒvYùÀ< C~ÚÑr@ +ßâSG?öm9ôîT?Öç=¼N${?âX¼$@kªÃˆê@È]Rkˆ¿î™‹âvØ$?ïþT>p©
¿Ý¢¼'ý¡¿Ëvh›ŸÙ¿æä:ýöe¿ðAGNbllRX J1233.0+1701?ïüáª/?Aqg9"??8õÖåŒ-?Aqg9"?ïԟgõîÀ?…,ð褳?u°L–ƒ¿?…,ð褳?ï…l*mc?†¯åû
ç~?Ž¤õo»?†¯åû
ç~?ï£Ë)g5!?n›M?x6Û?‡
5¦2·Á?n›M?x6Û?ï÷o@]Eß?U®¶"o£G?Q!fp'?U®¶"o£G?ï‰ñÇÜg?˜\náw8M?ƒº[ÇV4?˜\náw8M?ï"#\Õ²?‹"n§ë?Ž÷(ò»¿v?‹"n§ë?îøE
Ñ#ô?á6'6ž£? {¯¢=¾?á6'6ž£AGN4FGL J1233.6+5027¿Öâóç]@P›'ÿÀ:¼pøŸöÀ<¨~–ÞÔ6@€ïW¼)'@ÑyÚ·q?ÄÈñ¶f.?Ä·©º,?ýˆ¨°Ò@³§<ðK?ï¿ÜŽá¯³¿Ý#¶]ÞØ¿çJ¶!œÁ¿ç´Uý¸}
¿è,œ2¿ïÿÿ)@k*AGNbllTXS 1231+507?ïóãxώb?S'õE@kË?X9X¤,(?S'õE@kË?￘l{†è?''t]©å%?€äÕǐ*?''t]©å%?ï™'.ÿ--?†¿´OAJ'?‰¶4Jƒˆ•?†¿´OAJ'?ï
Ž\WLv?òiäñH?ž®4vÎ?H?òiäñH?ﲷ́ñ?"'M9Ô?ƒ~R	ñÛ?"'M9Ô?î²¢Þ«‹M?¨µl9ãFN?¤ÕÒׯ.?¨µl9ãFN?îÑK%‡?¡Ü&! æI?®"ëJ7òæ?¡Ü&! æI?ꍲZ°¦?¨±áÏh]Œ?ǍÉ6•=i?¨±áÏh]ŒAGN4FGL J1233.7-0144?·‹É#)bÀ@Nhj¹¦À9@'üí&	À<ð'Íó@ðGÙÞX:@a̾Šë?«'Ìx"n?‰ÇcEj\?ÝG¡Ÿw@
î /àÃO¿âù&Çë¿ä,ggfN¿àÊ1|yÎ"¿àî…ÿ³ÔÙ¿àÚßI§ÿ¿ß§†¡ð*JAGNbll3FGL J1233.7-0145NVSS J123341-014426?ïþ;±ÔE^?À'X)ƒ¯?,Dßh¤v?À'X)ƒ¯?ïô•:†±?[‡eç«?VՊÉb®"?[‡eç«?ïöÄ <Ë?`tê5²ü?Rw¿PΩ»?`tê5²ü?ïû½¨9?1cžÅÂñÙ?A	^Åø³V?1cžÅÂñÙ?ïý"Æ\"ô?)œIh\?6éÍûè×?)œIh\?ïÇZ'GÀ´?‡'"žzWt?|R¶ò%ï?‡'"žzWt?ïøÂú;?T´—{üŸ?LôÀÄ1o?T´—{üŸ?ïöÑDέ?He-ºêbÕ?R]vzô?He-ºêbÕAGN4FGL J1234.0-5735?ámúXe
µ@É°$öYŽÀ9 ø«wèoÀ;¡Ç¯VšA@jª›6Ó?ý1úNX?³…	>Ã	U?Àú¤ÌR©@œZz@	…™0=4"¿ïùw»"€^?ïâY'kÍ®¿ÕpB½ê±º¿Ýa%^ß3'¿Þèê8v¿å=»ýœ£dAGNbcu3FGL J1233.9-5736AT20G J123407-573552?ïü˜
l>?41¿ð?%^?;?" W?41¿ð?%^?ï"ëÀ`‹d?'™É
­¿?‹Ú·)?'™É
­¿?ïÏ<Ս*?z']=¡äÕ?xáŽZ3C?z']=¡äÕ?ï½D©¿*?cÿ"Ü®´¹?€®Õ¹°
m?cÿ"Ü®´¹?ïê|¤E?g+Qa¤d>?epƒS¼ª"?g+Qa¤d>?ìHhŒ‡?ŠK,z?½¿,»ŸÓÅ?ŠK,z?ïia¦õ3?'r;0؏ú?'ÓË25"?'r;0؏ú?î¡XžìX?'q¥ ðÂI?¥êv^0?'q¥ ðÂIAGN4FGL J1234.7-0434?îü ÷©;Å@MWS£ìÀ:ó¥S?ÏÀ<}ÊÞ)@ 9훤`È@|ˆGä?²——`Ú¿Šu¨Î•Ï¶?ÈXŒÞö#@ϗ‰!S?àHLŸëÃ2¿×õp¥.£,¿ãæ~¤ ´¿åy0}¡@'¿Èüªµöœ¿ÞŽ{·AGNbcu3FGL J1234.7-0437NVSS J123444-043623?ïþ¤Q>È#?šãϏÑ?%ºì-á6@?šãϏÑ?ïôbÏ_??ZzJí6Á2?W:b9v'Z?ZzJí6Á2?ïôûÛ÷?QÑÜ.©0œ?V	ùàJ'Ô?QÑÜ.©0œ?ïýÈ×A#?†.ñ1z?1¿€²Æ¦?†.ñ1z?ïüijgË?4'êhµ¿I?9Úc!±*X?4'êhµ¿I?ïÅÛ¨¡Ž?"‡ª"ú´£?}+ʵК?"‡ª"ú´£?ïôOÁšzÑ?e—u_Ð
Ÿ?W`|¬Íͯ?e—u_Ð
Ÿ?ïõÖh.à?HcjŠ›Ž?TSÛ¥ÔϞ?HcjŠ›ŽAGN4FGL J1236.3+3858?Èúøaٗi@SoŽ`€sÀ:Ç{ÿTßUÀ<¶=Y&âÃ@íçÈ%É@`¡F6E?½Ša~†Sþ¿¥ ÿ‡?é؋Fð@/UÌ¿îîεY+?ÑW:Ä¢ú¿âé³ÊG¿ÞâʚÃeE¿Ûä×E Æt¿Ð5ÂY¬CÀAGNbll3FGL J1236.6+3901RX J1236.4+3859?ïþÛÝXW§?*ú%Ò?"B'mÞO?*ú%Ò?ïöŠp†Ð¿?YiÈC«D?Rë‰êbR?YiÈC«D?ï÷èjž?­?U¥mÈ´Õ?P/*š‹µ?U¥mÈ´Õ?ïø©÷Mn?2ìòTRòŽ?MY»;W͝?2ìòTRòŽ?ïý—^Å¡ú?/Ëû¨ùë?3E›ÆÄê?/Ëû¨ùë?ïܖÓZtZ?y…éŒÁ±ö?q´–is??y…éŒÁ±ö?ïö{҉OJ?gæ`ҔÁ$?S[[Tì??gæ`ҔÁ$?ïÞÔ@€ðù?`ÍAÿ¹:?p•ß½w¿´?`ÍAÿ¹:AGN4FGL J1236.9-7232?ï¦i‹´ÕÀ#bÀh ÓÀ:~¸–ž=À< ÕÓËò@3òA{ul@Øâý¹÷?È=~æ»?ÂØgµ›Ø¹?ý‡†Œv›h?üy6ð'®?ïÿ–¹‰$¿ç=¾Q‰à¿çw!r–u¿â=n€¿çç]<9A¿ïÿQ÷GËAGNrdgPKS 1234-723?ïõ­E?Q͎W2ú#?UÒÒ?Q͎W2ú#?ïRRxò)?›æa'ض0?•µ°ú©ìÝ?›æa'ض0?ïÃж€?z%Ço'ƒ?~¤×NQ»?z%Ço'ƒ?ï"z¿Êìß?w¥X|áW"?›°¨
?w¥X|áW"?ïÁ
€¾xÄ?}h0><?y?«Â^/?}h0><?ì±Û04?À{´ÚgÀ?¿ÚwI&~^?À{´ÚgÀ?î/cMe†?£èGDÂe?­	Ë.1Ù¦?£èGDÂe?èdáU'P?­~ÊBPSø?Îlz©¶¿'?­~ÊBPSøAGN4FGL J1237.0+3019¿îfµª'†>@U`‡~äâmÀ;Ú¶\GÿsÀ<ëCòž@#<Ï8ŒäT?Ѭû¡ ¢?ä9ÓÀÝ?ïÿÐß´0@Œ•¥RÝ?ùl@ûÉ?ïÙÓ`dĦ¿ï;üR?íÐÇÎ`Jÿïì%W¨]'?ïæÑÆ0ÑY¿à¥è'%1AGNbllRX J1237.0+3020?ïõ ®¿N=?f‹ü4Îÿ?T¾¢Oé&ì?f‹ü4Îÿ?勉H¹¥?«±Lÿè!?…ü4°ÎÏ?«±Lÿè!?íX€‹;ï?£g†öú~Ô?µ;û¥²"ƒ?£g†öú~Ô?ïÛ6k¶‹?qç¿Õ‹â?rdÊQÁÂn?qç¿Õ‹â?ïç|Æ¥y?‰ø&‹½µn?hƒ9M,[?‰ø&‹½µn?î
õ|÷Õî?Ã!ñ×É*+?¯P¨3ò="?Ã!ñ×É*+?íS½˜ìu?£ÿ—ôxÄ?µb7Ã¥W?£ÿ—ôxÄ?ïÀ!¿S£§?‡GT*ä*?ï TÎT]?‡GT*ä*AGN4FGL J1237.8+6256?ïÞf"Mn7@KåâGˆUÀ;¢Qó蚉À=
]Qï@!Ã1Ãq"?ÿ#¶¾mŽ?ÊZˆâ'0𿧓¡2OB?Ùxœÿ§€@A#ݪÀˆ¿ÞGAÝðá¿èðk¢æIv¿æñ?Þ<`Ù¿Ïøö¡]¿Ø´^a4Me¿ÝùÚ·qõAGNbll3FGL J1237.9+62581H 1241+626?ïÿ1ÕK\±?ühÀxÜ?Å\Ûã?ühÀxÜ?ï÷©"ZâÇ?S0®¬üÑæ?P¬Öï"Â{?S0®¬üÑæ?ïèáè4?z¦Û§S<"?gû¤¼y?z¦Û§S<"?ïþ˜Àðdp?cgO{?&síÙG1Î?cgO{?ïÿ¬\ƒ¨Z?WúøfpÀ?èÒC5´`?WúøfpÀ?ïà´Ïï°Á?pÿÌ2Ûæ?oK/íó&í?pÿÌ2Ûæ?ïô?À4c	?sn)!6."?W€7Þh?sn)!6."?ïù¬ÍAÖ??KÐȬ?JLDGöÃ??KÐȬAGN4FGL J1238.1-4541?Ýÿ9‰Â¿@1df±æÀ:¡•ç]rÀ<MI)>¾@â
?#@*k
•?¹ÞÂÿª«Ì?µ b‹l?ùú>¥W<þ@"Ô§äá¿íÝ.^¸<?Êk|»<'¿ã€.Ä8©•¿âÆ®¥šXÜ¿à߸aÛ½+¿ïþE`zîAGNbll3FGL J1238.3-4543PMN J1238-4541?ïþY˜ˆÞ?rIf_¿?*ftç-?rIf_¿?ïè¥÷(ž?oa{¹¢Œ?gZûb|?oa{¹¢Œ?ïï'0¬¬W?fð…&`?`ØÏWs0Þ?fð…&`?ïú²Ï±¿¼?.`qa(4ö?E4À‰£?.`qa(4ö?ïýb''ŠE?/
jy¤1Ÿ?4ëjR©)ë?/
jy¤1Ÿ?ïðÿmD7?•¼`ï‹?ƒÀ+Ž*#?•¼`ï‹?ïé;»B?së³Þj?fæÄ;
&?së³Þj?ï뤦	‹ç?Uv²1hŸ?d[YëuXÃ?Uv²1hŸAGN4FGL J1238.3-1959¿î–'N£|@Eb´·,Q˜À9¨ÔÈCÑÀ<>÷ÂCÜÏ@BÙ¿¤p7@Ǟà*w£?³j·?-"´?­FæÄD½õ?øcì8¢Þ½@
JGB‰½Y¿½:ÙoÈdÞ¿à`ö…,û¿á݇?Nõ\¿á­%!ͅ.¿êöM½øô?¹ðCŸgAGNbll3FGL J1238.2-1958PMN J1238-1959?ïû/?6k(©Æª?CC"&'×?6k(©Æª?ïôUHBE?Xòª–éÔV?WUoN•©?Xòª–éÔV?ï£ÅwC‰?‰Z"֦̍?‡¢+ÏÁ¾?‰Z"֦̍?ïù¯³%J¬?8oæ<Wá
?IA2ñVSž?8oæ<Wá
?ïóQÐú{S?RÑÜyè¢4?Y\^&†9†?RÑÜyè¢4?ïÊ	›àÝ?™rx­ì?zû2S©e?™rx­ì?ïpÐÿ{9¡?'|*š`?'åà/ÑÕ?'|*š`?ïî	¦z†7?Tõ[|t?aöYÇrI?Tõ[|tAGN4FGL J1238.5-1201¿ëÈÓ¥Gçd@I[ë[-M@À9{[ùûÚÀ<&=:óñÕ@	T¦ h@@휻	h?³c%ên?°oÁÙԝ&?õ1\#…@µòοT¿ØOãÖԎ¿äþ§°³'¿çõ²JÃÉ¿é2µßËW,¿îAy¢XZ	¿ïÿí )k3AGNfsrq3FGL J1239.1-1158TXS 1235-117?ïý(JT•Œ?CZ¯ìNŸŒ?6½®
*²?CZ¯ìNŸŒ?ï󠉀zl?^wµ³T?X¾ì©Ô׶?^wµ³T?ïä¾zÆçþ?a'ÌÇJk?kA…H6J?a'ÌÇJk?ïþ¢¥[ï•?ûãúrœ?%Õ§qò
ó?ûãúrœ?ïþ³'ßÿì? 
ÜAÕ¯G?$ÇÑõ†z? 
ÜAÕ¯G?ïÊELL›?ý*§
Rå?zÝ@F›â ?ý*§
Rå?ïä".S$•?q,©a~?kÝÑ®;BÈ?q,©a~?ïü~‡´-³?6¹µ?<ÂUƘe?6¹µAGN4FGL J1239.4+0728?ÙÏweÖã@@QˆÕ¥¹bÀ:;q¿_üÀÀ<lTdÏ@;݂|œ‰@èÿI Û?ÁfbàtõJ?¿˜á7èύ?öIãxà¼@%U-¥?ïù+
ÊÄ¿ÑÅJâÒG¶¿Ýò
ƒÌ'á¿æŠ=²èö¿çs[wN¿ÐÞÒn¥ÐAGNbll3FGL J1239.4+0727PKS 1236+077?ïúŠãHdH?<c&Ï'?EÔqÒ³¸?<c&Ï'?ïçÄò…:‰?kàÊÔNÊ1?h;
¡Aj?kàÊÔNÊ1?ïà¿ûØþß?r'
ù.?o@øFpý?r'
ù.?ï¸$búí?h¦%gM¥?öç5­X¸?h¦%gM¥?ïÜ\â%›è?p?i§¼…?qюÞïï?p?i§¼…?ï¬&{P?Œ)8l>?"û~›è?Œ)8l>?ï !^'0N?Št
õ¯1?‡÷¨hu|‡?Št
õ¯1?îçogà©?‹}2vBÿ
?¡‰	'iÃj?‹}2vBÿ
AGN4FGL J1239.5+0443?ïǚzVç@PÚôðØDÐÀ7†¸
"'rÀ;q'¬?Ž‹@àðfÚÕy@Ò¢§_U?—ê&yçL«?¿–ˆÌAâ@%|Q£"î@­ï"ã?Ð>ý'¿ázÌ_¶Á¿å%)œ±|¿æŠ ˆK>¿ì«»Û
p¿ðAGNfsrq3FGL J1239.5+0443MG1 J123931+0443?ïǜVK¼?xáÈás‹ˆ?|1þ6'?xáÈás‹ˆ?ï±âÂż?¡î
Çõ›¥?ƒ‡O"=?¡î
Çõ›¥?íLñe»ú?§&+؈Þ/?µ˜tÐÖTˆ?§&+؈Þ/?ïêœg:‡÷?aª²
?ec˜Ó6x?aª²
?ï€Xw\Ð2?Œq<[º‹¹?éâ(Ëó€?Œq<[º‹¹?îû‰ßÎm?¼ü"a ?¦ Gd–Î%?¼ü"a ?îÓu_¸?š5DêLJß?¢ÈªOÒ}?š5DêLJß?ïIEõ
a6?ŠŒ¼ý¦þ??–×A\üR?ŠŒ¼ý¦þ?AGN4FGL J1240.1-6846?îjÓ§¦À²-"wú
À9à§7EÀ;çÇc×?í@ËÁPAáÍ@—Yûô؅?½Ñ¾¿?¶ÙþŸ¾ÝÝ?úCŠc›°Ë@ʯ‰ˆ¿à2Æü©3k¿Ý95@S­&¿æj]¡›Æ›¿âˆ?)5®¿äEœAi¬Â¿ïûC"¦%AGNbcuPKS 1236-684?ïö&ŒÔÉ?IäÁ
Þ©~?S²æ­*¾m?IäÁ
Þ©~?ïÑãªfz?'ë€ñò?w+{o?'ë€ñò?ïÉõf–Yk?z-BWº8b?{LÒ_î†?z-BWº8b?ïÉi¶'ô?^¤´>?{K$ڕŽM?^¤´>?ï҃ÒKև?m$òzBQ?v¾ÁWŒ¦?m$òzBQ?îßã4Ã+8?ª£¾/¬ê$?¢Ì·<èu?ª£¾/¬ê$?î͊±c(³?%¤	B?£'Tè¦Ñ?%¤	B?î'NŒï«ä?—O;Xn÷?­‹1á(Ã?—O;Xn÷AGN4FGL J1240.4-2606¿ÅkPG¸rÅ@BXc{ÐZ÷À:Ž£n.²À<;/•Y@€žBöŸ¯@¾¥<e?ÑFÆÞOâ?ÐÍž§ö?ûióžÈ­ƒ@¤­Q'Ñ?îê£aï^G¿æFGhÊ¿à×è‰ÁµB¿ßöÉàß(o¿ïÿùµc#¼¿ätü–¾óÆAGNbcuPMN J1240-2608?ïiŠD‰iB?'·½t~ÒÐ?'ηu²°?'·½t~ÒÐ?ïÌ vFr?uÑ╞ӹ?y¯ÄÕ7ς?uÑ╞ӹ?îúzã~?ZÚ·´W? XQĦŠ.?ZÚ·´W?ïU¦ûyU?uç;b*?•G«Ùc?uç;b*?îFiË0ý?¨.¸Š•ð?«žÙ_ÝT<?¨.¸Š•ð?ïP;¡|ù?˜Äº¢Ü?•ü؄ñ(è?˜Äº¢Ü?ì7L"vP?©GÅ5…œ,?¾EŸSdM?©GÅ5…œ,?ì´Ï—â?œ¦jýÉÑ?ºYë@ïù?œ¦jýÉÑAGN4FGL J1240.4-7148?ì~/©Ìþ²À!ì´®ÈÕÇÀ9y=07FÀ<¤—ú])@ µß5°)?ýì
Š,>L?²'s°Pë*?—¥bzž¶?鍎]ü4™?ýÊâlFOE?ïö¯¿uÌ5?ì|c}ÓÀ\¿åÇ´_¾¿ÖÚ"zx—¿ÔŸ
â@ÒX¿äʤ~z|AGNbcu3FGL J1240.3-71492MASS J12402118-7148578?ïøjŸRŽ?Isl´–?NU'¶V…$?Isl´–?ïß<ù':?tšV×ôè?paƒiÆ÷?tšV×ôè?ïÉï.ÃÚ,?}*d?‹)k?{hæý?}*d?‹)k?­ï±?xźS‰±?‹"s‡À?xźS‰±?ïñ¢žóB$?Sæºú»?\ºÁýþØj?Sæºú»?ï'b#^	?˜S
ÑÛ£?‹gw)úqÃ?˜S
ÑÛ£?ï¸)+#D?ƒ&Œºð¢±?õ¿¥?ƒ&Œºð¢±?î³MeʛU?—ºÆpÐ?¤Ë)¦Åæ¤?—ºÆpÐAGN4FGL J1241.3+4236¿à…ÏƸqÝ@R˜Äq´xBÀ;²íþu¼À<¸M_.cÁ@ƒÔª;Ó@@Q8¢ý%?Åø\]#¹?Æ´¯Êˆ?Ï"jãù#?ü·»á2?Ó¤ —@¿ØÌÅ@'¿ê¸ÅCk›¿ïùϚ¦ã?ïÆìž#l¿ïÿþBe«+AGNbcuB3 1239+429?ïö#n€L}?73¼Ó¬ü?S¹#å&f?73¼Ó¬ü?ïõ飸?YB_*!Ý?UÐ-;	Þ×?YB_*!Ý?ïeMuàD?‹ÂmR‡Å?"VQG$¿˜?‹ÂmR‡Å?ïþ´Õ£úµ?á僰p/?$²¨9¦@¸?á僰p/?ïî7è=…`?d¯"šò"´?aȤ>¿?d¯"šò"´?ïÒ¬Õásx?y ܳð?v©•WH?y ܳð?îÄùšÇRK?™Úˆª¼Š=?£°fQÓ
W?™Úˆª¼Š=?ïæØX¾y?mf¦²nÃ%?i'§	&îÏ?mf¦²nÃ%AGN4FGL J1241.5+3439?ïÀ}wéµ@TŒ
Ã7!ÕÀ;'ë£Q©@À<¼tªÌÈ@ ŠõíØ?ÿ5۞÷§l?Äöš;*""¿—»£К?Ԕy^»¢-@|Bÿ*Ø¿ï´4_®t?î©ýýÇA¿åwø_!·¿ÄæËümNb¿ç†´ð75 ¿¿•°ÖÍÏAGNbllRX J1241.6+3440?ïÿqoƒñg?8±'Z—?Ò®_h?8±'Z—?ï÷ôüŸUú?PË´š	)Â?P[Y>³?PË´š	)Â?ïõê-cn?V"	;÷R¶?T+¤Ð¯²l?V"	;÷R¶?ï÷Ò>Nš?8[Zè8þ?P[µ#‰ž?8[Zè8þ?ïÿ@!$µ8?ÆTXŽ`?ûÚóëi7?ÆTXŽ`?ïÞ³ãX?w\Í^âH?pø%ðÇTE?w\Í^âH?ïô6ý±àÒ?cœož[½Æ?W'0›V?cœož[½Æ?ï᜸2?bm	Æ
çi?ncGèòÕ?bm	Æ
çiAGN4FGL J1241.8-1456¿á	t۟"›@GïAcwžÀ:$ÝpˆÿÀ<D¨ª®•@ 2J*°°?û3	wx¢?Á#øÙÉà?Æpè géô@8Œ{£åM@då²ÌÆ?ïï›2öÍ¿åhrû?»"íe»þ¿Óc҂™Lî¿çÏ÷Å¶¿Å	ä˜ AGNbll3FGL J1241.6-1456RX J1241.8-1455?ïù1zÿÙ?HÜg㳇Î?Kç:3ãaÉ?HÜg㳇Î?ïޛ$ø̟?rˆ<;ÚÌ?p²m vhv?rˆ<;ÚÌ?ïé÷6$L?dàC­ÿÎ?fñœ€ÜŽ?dàC­ÿÎ?ïàjøÛ?qíՋ+OŒ?‹Çåtrõi?qíՋ+OŒ?ïì×2±??`ÉçHÝÂ#?c(ÎIÁ6?`ÉçHÝÂ#?°ýñ?™3œf\é?Œ"0Ó?™3œf\é?ï‡øý'LK?ŒÖAj®t?ŽÀ¢Ü‰9?ŒÖAj®t?…"ŽÆ?Ž~¿jçê?¥å7ªJȤ?Ž~¿jçêAGN4FGL J1241.9+0636?âû­3¨é@QV'è},|À;]Å~ú±âÀ<¹4@€@!#AúÌ9?ÖcÜþô_?âÞJ¹a¶?ïÿwTV™@KƧïž@'™Hæά¿îáóFí$¿à.ŠÂfA}¿ê8¨½ùË3?¬!
ä­š¿Ú'¾1(—¿ðAGNbll3FGL J1241.9+06391ES 1239+069?ï샛wâ‡?q"EÓ«"š?c|d‰}Pè?q"EÓ«"š?ïñ*M.J?dšÌ³ÆL?]«fLŒ5?dšÌ³ÆL?îÓ­ýk"?˜|‡·…B?¢Å.¿M`Æ?˜|‡·…B?ïø(Æòæ?BŽñÞËÆ?O_˜bv]É?BŽñÞËÆ?ïïÄÚ¡1û?h¬Å-?`;%oL%_?h¬Å-?ïºjcî^d?e<j z?efö©öü?e<j z?ïEAŽÑЩ?"Øß]PÆ ?—WÎ.\ðØ?"Øß]PÆ ?ïô¦°ƒk?aDcÉáZ'?V²žu8ø­?aDcÉáZ'AGN4FGL J1242.4-2948?áˆv¬.ǔ@@'-VÀ:ˆ<Ž%ÈÀ<7Cÿ3Qf@ìGÅ•Ï@@OÁß?ÐUŸÚ%zä?Ë9{â#¡?÷	f±@±¨‡s&¿ÀŸRK–¬¿èX;•ØCù¿ëukò—a±¿ïü"J|ûÔ¿ïªH]¼ÉŸ?§c¨¾GhAGNfsrqPKS 1240-294?ï뱸Z‹"?dV£ÖOS?dNG¢µ-ë?dV£ÖOS?ï±Sétç?ž˜Eñ Ë?ƒ«¶ÓG?ž˜Eñ Ë?ï5:mþÏî?Ž¿ÁŽèè?™X²G:6?Ž¿ÁŽèè?ïÍðä.=U?bç'•'ó;?y×³Iˆ?bç'•'ó;?ﬓ¨­¢?‰M&ÞÂí?"ÛÊHŒV?‰M&ÞÂí?íAiBþq#?¿w¹¨‹W•?µôµéÄDâ?¿w¹¨‹W•?ìyIGUL?©°› §LW?¼5´ÅU¤?©°› §LW?í+†U'y\?§c-á_Œö?¶£ÍSâ(Ÿ?§c-á_ŒöAGN4FGL J1242.6+7635¿Þ6‰ë%Ó@DCÿÞr¿À<ºSM"îÀ=2ŠÙã5Å@"o»'!­Ð?ú%kå+hd?Љ
uZ ?­öœ)øæ?ၽí@?ýɸl«¿¤· YfÏ?çïMËdíÀ?Ñö?âÄý¿æÅ!²­<¿ÝÙôhI?ÒÅ0"åˆAGNbll1RXS J124231.4+763419?ïý«ë<
?9¯_ø&Eì?3'Ÿ·‡Ÿ[?9¯_ø&Eì?ïó=ü˜u?Z-ƔPèÑ?YɄoC5[?Z-ƔPèÑ?ï'/rçܦ?Œìæ\e½'?‹t#8Jf"?Œìæ\e½'?ïØD'ßž¿?^ë^?ËÑá?sݶtԔ?^ë^?ËÑá?ïýIÞµo?5šUÿóÒy?5±
ß{mQ?5šUÿóÒy?ïÎ÷(Ò?xÛëÂì?xôk–ôE?xÛëÂì?ïÅ»NRÑè?ƒdfcPx?}"X¶ú¤^?ƒdfcPx?ï…'‰SGÈ?kÝÒ'…?Ž¶ ß:?kÝÒ'…AGN4FGL J1242.9+7315¿Óïè
?ôã@Eí?)
»EÀ;.W˜mI¯À<ò],+6@ "q!€XU?ÿ¾ü)±ª? ªõ>¿£ð<àÓa^?às–V;@<¿á¬Ø¼?ïòÒO̲¿éÆ	>˜7¿ÐõDz®Fû¿ÖJªH=†s¿ä6¼ÿŸˆ¿Ï¥~ª*
–AGNbcuS5 1241+73?ïýÊön‡?#"μëq?1¯Áq!Ñ?#"μëq?ïöº	•o?QzÇNº?SȌeÇa«?QzÇNº?ïôå¢(*ä?Uºd2ãº?V4»_óHÍ?Uºd2ãº?ïåò°P?L©ND¶%?jï
zK$ˆ?L©ND¶%?ïýO$€?.?V?Øé½?7×ÍÖ/†?.?V?Øé½?ïڗ¡,q?q®'µñ|ü?r´r+J?l?q®'µñ|ü?ï÷¯VÐ)?cκî"üß?P¡S‰)]ì?cκî"üß?ï©-.©r?n´	;xá?…´¾'t?n´	;xáAGN4FGL J1243.0+3950¿Ç+dÕ1>@SKGyBÀ:ÓG:Q5À<–jùs@ûrC>n@ÍÓB1Ó¸?¿‡î`ñ1†?s—'ÝR8?±böð6ß:@tà*?ë—­µ°¿æ´:æ…Û¿é=Ú rfO¿è:ÑÂÕÓ¿ð?ïÿþó…õAGNbcuSDSS J124318.91+395117.7?ïÄaÙ¹Å3?¯zabÎ|?}ÏB	âB?¯zabÎ|?ïõhA)bq?W."Ca§?U/}pÁý?W."Ca§?ï'MH÷Ú[?ŒÃ_ÔG?l­´Jù7?ŒÃ_ÔG?ïáo‹u‹ë?`®…4œ?ntZYœ?`®…4œ?ïÃE+'B?‰±ÆnÌ­?~]j]þ£3?‰±ÆnÌ­?ïÍ¥H_¦j?Ëû'ëaÑ?y-[èéúä?Ëû'ëaÑ?ï¤icÆÎÜ?‰}ƒ—¯?†å¦ý=?‰}ƒ—¯?ï<EÍáí?'Ø@£}*ö?žxwFCÂ^?'Ø@£}*öAGN4FGL J1243.2+3627?à¦h¿Î•@T œ^o÷àÀ8d çk´"À;w²Ý7~@¸Á¾Ñ·m?úa
 ë2?£k/MöX?®#ÃöÝ@àj¾º»R@oÑ^¬Þ›?ï>S¯­'¿Ô^ßY—K¿Ùß͚ýòµ¿Ñeœ\AŸ]¿Þ"Þð¿ÛWQ`ñAGNbll3FGL J1243.1+3627Ton 116?ïîyÒvQ?YÇŽ9¤ž?ap†rAÞ>?YÇŽ9¤ž?ïïó(½J?ªýkÑ	rp?âžWòÅ?ªýkÑ	rp?ïozVˆLë?'â, ëõ?'µ5՚"?'â, ëõ?íüQþ-¦?"Ôbƍ‡?°pàÝK?"Ôbƍ‡?ïė?ˆgS?w™å¿Aå?}´`?²{?w™å¿Aå?ìók‹Ù|?Âð`ßÙ?¸d£ \%?Âð`ßÙ?ï]H\²ç?'"ÃN7µ?"VôbÐË-?'"ÃN7µ?é[ð'0?³«—A&p?˞?cÿ??³«—A&pAGN4FGL J1243.9-0218¿éðÓÎYü@NA	Ö¶[À:C(0 ±¼À<f/çCq@ðÒ]…l;@]°µ??Äv¹Å³þË?ǎ_ê o·@w¥ôïp@au¼o²j¿Ý<û ŸÈ¿çËÿÚ@S¿Ýæ"Cqò¿ß[é€Óô¿æצ
4¿ïós_s-AGNbcu3FGL J1243.9-0217PMN J1243-0218?ïúäæôì?BÚþ'ò¿?GðmeûM?BÚþ'ò¿?ïóhîèÜ?_(¾.1=?Y."±–ô?_(¾.1=?ïçöB'?p;	6!´?h	ìá"ØÞ?p;	6!´?ïü¢˜E܃?$²wÇ(ƒø?:ë?|Ѫû?$²wÇ(ƒø?ïûŸ¢a=?>]ð5©È›?Aw4w:?>]ð5©È›?ïÁ"¯[ ?1È1Ú?6(S+Ü2?1È1Ú?ïÈôºôÕw?€ôâ?ý¨V?{…¢eøÜ»?€ôâ?ý¨V?ï÷ï{M~?@wò&ëö?QÖ!iš
?@wò&ëöAGN4FGL J1244.2-4956?秊äiˆ@)Ҟ²N©À:‰XÀ<+©­
å@Ê	rðb~@öäÎ?¸¯¤@î?›C‹p*Ö?âª''¥@ÉbŠ
à¿Ì†9•w÷¿ãª3z€Ïž¿çŸÑâ5iÄ¿ßk*ñER¿äóý">5Æ¿á…\€‰}BAGNbcu3FGL J1244.3-4955SUMSS J124422-495422?ïýú9A•!?¹âêRØz?0.49V	j?¹âêRØz?ïë2֖û?p_a¼Áèq?dÍ)UÇ,Y?p_a¼Áèq?ïùõÙzI?732sœ/p?H(š©?732sœ/p?ïû_
7͈?)ÑÕúj–?BƒØ*R:?)ÑÕúj–?ïüÕò]?6®Lì» ??WÎb!?6®Lì» ?ïRé¸?¢°£¯ô¯'?•®BÌlûb?¢°£¯ô¯'?ï÷¡?]ìx?bæ é).?P½‹žïÆ?bæ é).?ïí3hÑê]?Re¾Þ"õ?b̗B³K?Re¾Þ"õAGN4FGL J1244.5+1616?ܛÄ-ä6B@SÂ=ÿ?àÀ:žÝõ<ôÀ<'è5Þß@l¦¿òÉ·@¨ _ñØ?»sLþ¶Så¿£1ÁKÂÕ?èIËÆ<Ó@€LÁz?í"ú¾z¿×9ƒ@;Ú¿áMÖ¸ª¿ãýR ^DY¿ÕïW¦°'¿åŒµ_ó°'AGNbll3FGL J1244.1+1615SDSS J124444.35+161621.7?ïø=MŠÄ·?@\‰w?O
É7²85?@\‰w?ïëvèáø¥?kM'•u5u?d‰ö+âÒ?kM'•u5u?ïæ†	¢s»?ešîïé‡Æ?iyöBdº?ešîïé‡Æ?ïßyð†æ9?V?5E?Më?pC²íû¶?V?5E?Më?ïܧ~gA¶?có®Ý©a?q¬@Înèâ?có®Ý©a?ï™ØuÄʗ?"Îuº€ð?‰‰â‡î"<?"Îuº€ð?ïÛ¤Àá~'?v¬>Ó ‰¡?r-Ÿ¡¶ã?v¬>Ó ‰¡?ïAëxşÃ?ˆÛ|+äN8?—çLž?ˆÛ|+äN8AGN4FGL J1245.1+5709?àx:¥Ý
¦@Mùˆ MÀ:>¢Œ‡b_À<¯è+Íä@‰€Ç»–@x\È_?»KË@ÁÍQ?¬ŠŸM/*?ñ××ârP@³£ùnìG?ïþÂ}¾qÀ¿Ø£k_I'™¿ãŽ.+ŒuÅ¿Ú~(Õ!°¿á©!âRðé¿ïÿâ¾÷!AGNbll3FGL J1244.8+57071RXS J124510.5+571020?ïýàZj§
?#ÿv¾Ö"?0ý*ã•
*?#ÿv¾Ö"?ï÷@wO¨ñ?Qvf
	g?Q4³|?Qvf
	g?ïðœØ	ä'?`Ä¿~¯Ú5?^ÆOéx^?`Ä¿~¯Ú5?ïèä»´,?OûÀ?gDfL‹?OûÀ?ïýߝù"p?(šxµÿΰ?1` ¦-?(šxµÿΰ?ïßòF·}
?q¾‡r´?pܳ_Án?q¾‡r´?ïçcE8ˆ!?t ¾×'ƒ?hœºð³/8?t ¾×'ƒ?ïÈÂbKàº?gçúM®?{žÎدÊÚ?gçúM®AGN4FGL J1245.8+0232¿Ù Ô¢j^Õ@PX4Á¨¬\À:ÒùXF3À<°·ŠEhÀ@‰Y"Eò¨@cIÙgåÂ?ÇҁÀá²?à©=EÛ¬d@U$¿ÒéG@-Äq3žé¿ïâ^¯c?ïEmþ
\z¿Ú!Ïþ°t§¿åÞ¯6'¿í8´FÄ	°¿ïýðƧÞAGNbllNVSS J124533+022825?ë»ènÇf?¾Ü&qƒÐÚ?Á^DâeÄ?¾Ü&qƒÐÚ?êÓzì/h£?Á4ŒÕ÷ÿè?IJOB]s?Á4ŒÕ÷ÿè?çoF¼IiM?³JÑg¬°¤?Ñ!r‡m-f?³JÑg¬°¤?ìˏæÅúÔ?˜ÖÞûKÛä?¹£€ÉÐ)_?˜ÖÞûKÛä?Ûó	ÄÇ<7?Ê ôc·?â{œaå?Ê ôc·?á!VÝ€Î?ÐÝÞ:þ?ݽREòþe?ÐÝÞ:þ?Ò¦:¤
2e?¸µÞ
"4Ð?æ¬â­ùfÎ?¸µÞ
"4Ð?Þ?¤I¯Ð?¸†§<?F?àà-Û8(?¸†§<?FMIXED4FGL J1246.3+0112¿" &ƒOêÊ@Pʽf'À;0íæ²QÀ<¦¦3
@ºþ‰³G–?ý*þE뜜?מքÜs3?ÎhìƒK?öz¬(©l@o…r›(¿æhŒEô¿æ¸Ã*Œœ¿ä÷'î\i¿Ä‹í¬vì¿åïw‡ R¿ïù}š_'7AGNbllPMN J1246+0113?ïþ@Uì¬Í?!;…4#•¡?+út:<?!;…4#•¡?ïñØL)EÁ?_RÊJv?\OgJ¾œ?_RÊJv?ïè? ôW?`ób?g­d?gÀülÊ?`ób?g­d?ïúmœu?,úa	SôM?FKÐõ.ð˜?,úa	SôM?ïÿDLqXï?¬îêoƒþ?vn!4?¬îêoƒþ?ïĈçßfœ?†ó‰'Î?}»Œ+éÞ?†ó‰'Î?ïëéá8GM?j1¯eãӇ?d"Þ{x?j1¯eãӇ?ïé>I´ {?YÛZ'Ð?fÁ¶&ýG?YÛZ'ÐAGN4FGL J1246.7-2548?ïþ¦b™—@B‡jƒ+™À7]M•µ‹À;>Ð}[ur@õ@Lz@¶ŸÜ©¹¢?"i†<«¾?¾îܗ8@'w,¶Ap
@ð‰JìãC¿Ê,jÈÌ¿àf¤^ïy ¿ä؅½™©	¿åÿdd-§¿çȽ¼
¸¿ï(	3…iAGNfsrq3FGL J1246.7-2547PKS 1244-255?ïðô÷ä'²?]âÝ+Pþ?^ߺ›ã?]âÝ+Pþ?îE#aȶ¬?µ«3àÅ6²?«­Éãt•9?µ«3àÅ6²?ï§~ò€¢?ˆ§1Àhüž?† y®«"?ˆ§1Àhüž?.¿Ÿ×?Š½Æÿ?Š´]Öz?Š½Æÿ?ïÓ)™g«Ç?QÙ€ƒ÷?vk3[Hdl?QÙ€ƒ÷?ç`Û<|2+?Ñp"é;÷?Ñ>I‡›«?Ñp"é;÷?ï§)¹{¦?Ì Œdî?†5'"Xu?Ì Œdî?êmv×çvá?¹o©"|u?ÆJ$ b$|?¹o©"|uAGN4FGL J1247.0+4421?ïРjTmÒ@R0
ú/§À:j1ί%À<}ËÆ<Ó@ T¸?ú+Ì¢¢&?Ââg=Ñdz?ÂsLhckµ@óþº…¢l@šˆÙ-m¿í3e"¤7¿È[QIô•¿¿Ø¬@»1ý¿ÐÑÑCſܨݤ‹e#¿âüê×yÎùAGNbll3FGL J1247.0+4421RX J1246.9+4423?ïþݨ¹?"…";Ã?".Èlòf?"…";Ã?ïô-:Œ¿?Y¶¢Åc‹9?W¥Šöäƒ?Y¶¢Åc‹9?ïõ%þ05í?VDä'Ú_?U´šÆè?VDä'Ú_?ï곌"ÒW?FÛs0ÿÒ?eLsÙ!G?FÛs0ÿÒ?ïû·Bhä?=(ƒx|£6?A#†ÏT6?=(ƒx|£6?ïÓ·¦[/7?{ŸS›÷*Ž?v$,µ‹¬¸?{ŸS›÷*Ž?ïñÖ4ÌÞ?f{Á5²?]îSIoÿ?f{Á5²?ï´õ~"?p&PÅÈÕ?'¿^ûe?p&PÅÈÕAGN4FGL J1248.3+5820¿×'æ{ì×Ò@McáÁP—ÈÀ7²ÂFbÀ;QDy¬"H@#'0iK?üù!ÚE[T?"ZýU­º?§]®1S@lë5m @²ŒI¥¿ºOOŸx+¿Ü[é B*G¿Ý­2=>ú½¿ÙŸÕ]jo¿áGßÝË¢«¿à;‹ÇHÿAGNbll3FGL J1248.2+5820PG 1246+586?ïýHênb"?1[£˜æ7?5¸¬{WUh?1[£˜æ7?ïñ]èéc?c\|ƒbc`?]D.««"??c\|ƒbc`?ïજ˜žê?t7pqP?oUc%h–)?t7pqP?ïá{+Uªh?X%´ú‰h?n"Ô̱°"?X%´ú‰h?ïþ4C(ž°?%ao‹È?,»Ðð¯ÀL?%ao‹È?ïÕÒi'5"?x¬Mû‡\˜?uË3E­Ù?x¬Mû‡\˜?ïæ³~OÄÂ?{¯_ISÀx?iL´ZÆ?{¯_ISÀx?ï©Ø	Rn?uQÍe¤#?…‰ýµÆø'?uQÍe¤#AGN4FGL J1248.7+5127¿Á-BÔ÷ú´@Pj:ÀÆ.MÀ:çÓƼ"À<Ö35·qò@ýV"U@sˆ€l¡ê?ÀOBßN…?  ÜÄf¢?Ðσ@;ÚL@ô%ä–.?ïúKUhè!¿æӀ y\¸¿Ømû:ôG»¿áTBý«'ê¿ä¬œ«¿Ð7h!&–BAGNbll3FGL J1248.0+5130RX J1248.4+5128?ïýuàñ‹¸?,·qÒ™?4Pö¨	·n?,·qÒ™?ïøÏùÒê?Pɐ ØBn?O"À
õæò?Pɐ ØBn?ï÷PÉ=˜‰?U»6fŠHÒ?Q^mf']Ÿ?U»6fŠHÒ?ïïÌRö¿\?DÀyŸë2D?`3­ ûò?DÀyŸë2D?ïüF??8µ	*"??ßf)Iî?8µ	*"?ïà# 
?q2f^Í£‰?oÜßøwBP?q2f^Í£‰?ï÷9?ð8•?açÍs§Ì?Q€›@ij?açÍs§Ì?ïÔ<PEñ/?`wNãaÌ?uá×ûóä?`wNãaÌAGN4FGL J1248.9+4840¿¬äbÄ!@Qý`éNäÀ:½´ò»sßÀ<Ã9W9¢¹@=x±"ø@2™åﳂ?ÂxÛ^?«
®e?çˆäu_þm@)Ùçg'Æ¿åfH3ux¿ãn¯«SÖA¿æýh@[9â¿áV¨ž[¿ïΗÝ×·¿ï׌CoÁYAGNbcu87GB 124632.9+485605?ïý–¥Á<?,¨_~vJ?3JÕÓK›?,¨_~vJ?ïøP7@6?PÕÂ}]4Ï?N¿$=$?PÕÂ}]4Ï?ïí‹G?Z"Öó3—F?bóáoaXÖ?Z"Öó3—F?ïüA€N'?+2óã'@?=÷¾
Or|?+2óã'@?ïý­úÆýw?/1‹Œ¿WK?2*ѽJ?/1‹Œ¿WK?ïß»ˆ=?s·Fu~¶?p";Õbv?s·Fu~¶?ïóÐCœ.l?e0Å,µå?X_xN°é?e0Å,µå?ïõ©6g?I:y¥ƒ,=?UЭ^÷Ìö?I:y¥ƒ,=AGN4FGL J1249.2-2809?ç8˜V'L¸@A\ÂzcÀ9óšw+À<J–6—l@4žm=ñ@/»õäô?¶ˆWQölÙ?¦
L46?ðÐÄ©Ü¡@!åÆüÌ¿âÚ%æC–X¿Ûhfç¿å&ýšÊò¿ÕŠJWu¿ã-ª}l'O¿áž¨âŒÒŒAGNbcu3FGL J1249.1-2808NVSS J124919-280833?ïþRÞž ?»1,í4?*×°È?»1,í4?ïóPrfØZ?Y­X¨Œ h?Y_«ž?Y­X¨Œ h?ïøy
ØÌ
?T>ºãYÃÎ?Nԋ8@q?T>ºãYÃÎ?ïö%ö™?:Ëä&—r'?S´f8ìú?:Ëä&—r'?ïýølôÜ?/ŠoD
?­?7 <¢>e{?/ŠoD
?­?ïÇòiXM
?€Ÿnö"ö–?|ËPiݑ?€Ÿnö"ö–?ïù šÕ-ï?_ŗ–5"=?K}•²Ç´?_ŗ–5"=?ïÚ§ÐWà€?`ÿNTûÈ¡?r¬ê½+¥?`ÿNTûÈ¡AGN4FGL J1249.3-0545?íëçH'Ú§@L"V!uÀ9ìfknããÀ<)ñʳ@°5;Ì	?þ°ÆÜÈÃS?Àßäׅ?¿|F¢{Àk?üðÁo¡y@
óÍ]ìDa?±–!êá_׿҃Û!#f7¿ázá}]ù°¿ÝèèŒEô¿àáMø±W&¿èååvø…AGNbcu3FGL J1249.5-0546GALEXASC J124919.46-054539.7?ïþ[=qT?"¾»²Û?*L-ÉÛû?"¾»²Û?ïñÌ®2È?b]jÐÁ–"?]ÆfûpW?b]jÐÁ–"?ïöèjÉ2Ë?@(ðÝdA[?R/*º'ªn?@(ðÝdA[?ïúE¶˜'î?/aÓCYR?Fé%ûöc"?/aÓCYR?ïúԄÒR??æj{׏?D­íö³??æj{׏?ïÁØT6ÛV?¹7Ú<?Õýÿpø?¹7Ú<?ïéiàUù?q§ÒÅ}?f–ȏ~Í?q§ÒÅ}?ïð²}žÄÚ?LM‹N?^›T'Ì?LM‹NAGN4FGL J1249.8+3707?ãñ—"h@Sÿ|E˼,À:5áŠëÀ<ZÝÌÏQ@ —øo'ßì?ú¤Ò—çè²?¾š½°û
"?»ÊkH£\ç?ùkøáþ9@v[»¹f?í÷G"êp¿ål­byFé¿Òv2â*'
¿ÆŸiýŸ¨|¿á¨[ý¿Ü'ÁM'AGNbll3FGL J1249.7+37052MASS J12494675+3707474?ïÿ#ë±XA?YKVy¤?'…-ÿ?YKVy¤?ï÷Õã»@?P[•Ødõ"?PUАÅÞ«?P[•Ødõ"?ïø¼:F?[Åtu"?M­Bò	?[Åtu"?ïõÈ7M|?<²
|§m?ToßFY#?<²
|§m?ïÿXa6?e"‹¡0—?î.Ö9?e"‹¡0—?ïߎð?»?s¸'ËT&?pv¸‡06…?s¸'ËT&?ïúñM_¯=?YÀћ°w?D:ɕ÷fy?YÀћ°w?ïî²ÔíÇ]?N€Kæ?aM*úÛK?N€KæAGN4FGL J1250.6+0217?åD,ÊZÎû@PJ%®æ1ùÀ:7Faä ¦À<[DÐêh¿@Ÿ0'ü?ÿéki¦X?½e?½I?µô'žUk?øՐÀ­Ú@¦û˽Ù?Ú¿†ÞV&?ß¡B‡N¿äƒõ¶6ˆ¿Ù­K6_¿åÍF¿×ñĿُ­‡'›AGNbll3FGL J1250.5+0217PKS 1247+025?ïúuÐDY)?:°av|?F(¾)ËVð?:°av|?ïÕôš,w¾?we—ù?u²äDÀÖ?we—ù?ïïlí>1i?b§K0D‰N?`"Ê
¦ñ?b§K0D‰N?ï'U'þ?pkшÕv?‹j¸ÞíÜs?pkшÕv?ïðب"H?VˆAÉ?^N¯nwÁÕ?VˆAÉ?ïq«§´º?"|$ŒÓí»?'ÊŸK	h´?"|$ŒÓí»?ïé:¼Çú‰?rÓÂ	"\,?fÅBüì/­?rÓÂ	"\,?îX½þ &?—€HKk?¯Jt ý¡?—€HKkAGN4FGL J1250.8+3117?Ü8¸`â¡@UuÎ1PÚäÀ:½^¿¨÷ÛÀ<³ùJ÷@½ënM'@dà?p?ň#û\Ø?ÀÇ`âÃÚ?ú4Q%Œƒ@—멱¿«?ïéæ]Â}é¿Êp¡Mm¿àÅîÁ껿çoñ)£g¿Ø§9ª€¿ïÿãzŽ;˜AGNbcuNVSS J125051+311706?ïþ%罋^?#¡åµð¹?-¡ƒ–'r?#¡åµð¹?ïõ"ßZ+?V¨ëš°?TØxíF¨Ó?V¨ëš°?ïë]>a¡?ak~#Šœ?d¢ëŠ¤ŸŒ?ak~#Šœ?ïè~?\G?Jõ}:çæÍ?gÀk^؆?Jõ}:çæÍ?ïúäsmÇ?AÎ2"?Dn1¶Ç?AÎ2"?ïÛhñYk?uºï1S«?rKð#þL?uºï1S«?ïÙDÛ.íÝ?wXÀ܌²?s]'l¨™˜?wXÀ܌²?ï©® DŒ*?rå"ÊýÁ?…"Wõ¼-Ž?rå"ÊýÁAGN4FGL J1251.2+1039?ÖÚjŽXÉ@Raž­ÕÁÀ:È_Ñ÷®ùÀ<Ûž ç×@å•á"@CLŠÅÁ?ÊC#–21?³Øj9ڗ;?êÿ'>‰(@y	ڛ?ÌöÄŸä¿éØS³Ü:ÿ¿Õ—zEˆÓ¿ßѾmþ¿äóUÝ­Ô¿ãØr¥®AGNbll3FGL J1251.3+10411RXS J125117.4+103914?ïœô5$?¸8bãs.*?ˆà8µ4G?¸8bãs.*?ïóŠnXx<?cB_¨ ?Xë#V?cB_¨ ?ïö¤æÇÃ?giƆL`Ý?R¶2Ëg©?giƆL`Ý?ïùß_Õ^?0­+62ø?H'€2øHN?0­+62ø?ïþþdÞH? °ù_Pۜ? »âÛ¶+? °ù_Pۜ?ïÎAç ?¡ßW£³Ù?xß]ô?¡ßW£³Ù?ïò½¡®‡?sÄÅGïl-?Z"¼ëhÑH?sÄÅGïl-?ïí'ÞRlp?Nn®8Bn*?b}!˜õèw?Nn®8Bn*AGN4FGL J1251.3-0201?Ñ®¹ÀšSB@Nl)Ür\À9çÆaxÀÜÀ< ªÍÛÁ@Wš©+½?ÿ5}?Æ¿m?·íå᛻Þ?Ãð\žçaN@
–Õ"õÎ@Ú\`ˆ×?îÃRЇlp?ÀÁûxö¿àÖ8¡1=¿ãh&à>™™¿è	 B*Fû¿Ü.]Á&PwAGNbcu3FGL J1251.0-0203TXS 1248-017?鱗VSôŸ?µb›Ú5?†jnrtH?µb›Ú5?ïïs˜~§?g4WÒM4ÿ?`Œgl8Ã?g4WÒM4ÿ?ï¹ÿAWýÝ?Ž²TåVO?€/™'hí?Ž²TåVO?ïùƒ•ò4?2E ‹~?Ió•!†€Â?2E ‹~?ïö-éÈ00?O§ƒûPî?S¤,ðÐïf?O§ƒûPî?ï»ñ±aU?Šnö3Ì«Ø?"¹×æÕ?Šnö3Ì«Ø?îòٜœ‹ð?–í–´{º? Òf8Êõþ?–í–´{º?ïîÑw'w?M-Îc£û?a.‰	ðÄ?M-Îc£ûAGN4FGL J1251.3-1719?К+¸žC@FÆ~¿"ÀÀ:ƒ½‹ç)À<0'½,EÙ@Œ½T´¸.@Rå=Ì?Åi ÕãvÝ¿¯C²¡To?æÈa-A'?ý"ˆ'ðਿã)ò­1&¿çôáSlŽŸ¿èÖ¨]¬®t¿ïÿþó…õ?ïÿ¬ž5¿¿ïÿ±%§YvAGNfsrqPMN J1251-1717?ïù®y?s1®Ê=†_?IFWuûÁ?s1®Ê=†_?ïëÝþ<JM?sw֐ñÛt?d"®2µ?sw֐ñÛt?îÙ½6Ãó?›‰y|Gî?¢d.k·ÙØ?›‰y|Gî?ïÿxæ=-ª?%:9'Ô?ã6ÇÞÞ?%:9'Ô?ïöòÚò?`/¿à }?Rà—1R?`/¿à }?ïUöž¤½±?¥D#5-A(?•A,&@ßÙ?¥D#5-A(?î‰ÃZ)¹"?cÙé÷È'?§cÊ]dg¼?cÙé÷È'?ïæs:pzx?ov˜Ó§"?iŒÅʞÐ?ov˜Ó§"AGN4FGL J1253.2+5301¿ïRCwàœ@Pö¾7ޔÀ8¢}À;`F'µ@F‰!|?þæ™&­ó?äè!'ö?¶Ža¯Ž@}4ßݵ@¨ªƒ¡¶¿´wù
îE˜¿ÓFšDšd¿àíA·Zu¿àVƒ?4{¿ä\¼>4C)¿äCëGWLAGNbll3FGL J1253.2+5300S4 1250+53?ïûêíw¬?D`®•UÏ4?@WÁ6†nØ?D`®•UÏ4?ïœGœ Ýp?›D§¦òO?ˆî‡à?›D§¦òO?ï·ìoíÏ?‡ß³É	Œ?'ùl›'K?‡ß³É	Œ?ïX4ƟûÍ?€3éðSψ?"ùg%!Nd?€3éðSψ?ïõȉÇ?`™èž5qé?UØnásÅ?`™èž5qé?îi*@p]‹?³7…‹Ú?©m[ýEªH?³7…‹Ú?ï¹WŽÿ"'?‰*–À9?ªN5\I?‰*–À9?ëµ8H=Ré?§À'®}?Á+ß
´[?§À'®}AGN4FGL J1253.5-3934¿Ëÿ8ÔKµû@7M‡ø‡eºÀ;Oô!¥l6À<­qGÏ¢@"RüÎÈ$œ?õ»
7 '¾?×(ª.'?ÞBãÈÂý@\ÝF—"@hU¥ÎÜ¿ääáÞ?¿ð?ð?Û襁6¿·d^ -¿æºÀZ΂¯AGNbll1RXS J125341.2-393200?ïþùÁ¢w?'®1'z¥È?.fÎ<¸?'®1'z¥È?ïîﺖ?b±šõê?aE0*|?b±šõê?ïÇÞEÆâ?ux Æ?|Ý
<?ux Æ?ïøì¤È:±?@ËÙÐ4\?LMl&ê.˜?@ËÙÐ4\?ïýÃw"?.,|Td¡¨?1äH71<?.,|Td¡¨?ï¸S7×Õ?…B†Éud?ë2';:?…B†Éud?ïÜAÏ®(?z}Ç["À?qßìñ¤?z}Ç["À?ïîàÜ+íø?]Nþòåt?a#H.?]NþòåtAGN4FGL J1253.8+0327¿îMv
"z@P"3œ¾àÀ9vZT	lÀ<á¦x¥-@—˜épq'?þ¨S¦pA±?²\[J©q~?²ï'ó²ê£@ºÆ:"‰@ÂÂ¥V'1?ïæfÁ«¨¿Þlâ×P3¿ØÙL!–¨£¿âñµºa¿àajþütÛ¿ãIsÔ
3AGNbll3FGL J1253.7+0327MG1 J125348+0326?ïýýP)7?§?]§âë?0€˜û­-?§?]§âë?ïèãõ?n$s›»ÚM?g
ßl` ?n$s›»ÚM?ïñJÃʁ?eMzÜf-?]kôÓ ­Û?eMzÜf-?ïŀŸš?d ©£:ùÄ?}?°JZI&?d ©£:ùÄ?ïû;¾®7G?6¡éd·?C)?6¡éd·?ï´óÙdè?‡=©P=Q'?'Ã	¿aÞ?‡=©P=Q'?ïèúÕÉ ?rê@vjb?g*#!'¬?rê@vjb?ïFÆÇ`b}?"A¿"ç
F?—''
xy?"A¿"ç
FAGN4FGL J1253.8+6242¿ïì­îg§@K5ܜM©À:YÜë(À<Ÿ!ÿ.Hé@ì˕j5?ÿRþûB0?³Dç­†?—qd¤ÍÝÍ?ä
*àÔ@´@»ù¨M?ï§0ü!N.¿â®¡Óú¾x¿àý¢È6¿Øó"
3`¿ä¾‡Å[¿C¿Ú†«ë«µ%AGNbll3FGL J1254.1+62401RXS J125400.1+624303?ïôŽÈ¸É"?"}¬Eq7ö?Vânña™?"}¬Eq7ö?ïøÉ¡/vK?Oû¶lç-4?LÙz'®`?Oû¶lç-4?ïúqœêÞ?3æ|J;™j?F9ŒûLÑ?3æ|J;™j?ïü'™Þ??+<õ¬ÀÝV?>Ã/çIB€?+<õ¬ÀÝV?ïþ?žÙýë?&Lºðíud?,©qQ$?&Lºðíud?ïá#@Ýý?p‰E¸jÅê?nùÜþZÒÌ?p‰E¸jÅê?ïú¶nUaö?[lr£B[6?E&FÏÚN&?[lr£B[6?ïú¼­"–?5	Ì8Xc?E
K`7e?5	Ì8XcAGN4FGL J1253.8+2929¿í¹k½NÃ@Uä‡Tów\À;¦JœÜDÀ<èdØǬÒ@ —aºH9?ô‡™Sù?à?…¡•ž?ÕÜ%³î¯?ó¬õ–ðqî@ Ü&$?ïúÁ.ˆÿ¿ïÌ{n5gÁ?è¨+b"Y–¿ÎfÆÞvB|¿áŸÂ¨†œ¿à×QÄòAGNbcuFIRST J125405.0+292708?ïø_ōh^?BRI
Z‹?N€ê"·`?BRI
Z‹?ïôµ¤B?]ÿ‹iiÌ?Wҕ#KÞ?]ÿ‹iiÌ?ï¹°v¡¾?€ÓšÜ6ºŽ?"â‹Ö‹?€ÓšÜ6ºŽ?ïÙgK#ûï?]i²³]pb?sLZQÕ<·?]i²³]pb?ïúŒõhÅ?Doi™(?FÌ4B3'?Doi™(?ïÛ4j¦ù?{w—_Y?rse«¤?{w—_Y?ïÝ┒Ò3?võѯ`Y?qµÒÆw?võѯ`Y?ïÎËf_b?n)aÎÖ*,?xšL읚¬?n)aÎÖ*,AGN4FGL J1254.2-2205¿â{¸²…ñ@DcÖ¶Zš€À:I}.ÿÇÌÀ<HéH-–;@g:<fã@	ýñ7?DZÓ!O°í?Èðužg´š?ÿ|卍ó@
Ÿ˜^†;?íŸ9Q´~¿Ý¯Òò䏿â0"刿àµ{!	¿åI¾ RÔ¿ïÒÁ££Þ—AGNbcu3FGL J1254.1-2203NVSS J125422-220413?ïù15ÆÐ"?A½Ì¥¹?K;)Eó?A½Ì¥¹?ïòðË.½?WݵN•2?Zi"ý?WݵN•2?ïç+ô¶±ê?jڀÔx«?hÔQ&r?jڀÔx«?ïíyå
$E?C[x'¤_k?b†ԟ+?C[x'¤_k?ïøÌdȵ?F'³À‹œ¾?LÎmsߍŸ?F'³À‹œ¾?ï¼¥Êvӓ?•«Äè{?€Öl™ï?•«Äè{?[ºÞ/?ŠÄ­é¿?‡é"v€?ŠÄ­é¿?ïÃèl\ìâ?d7b't†?~ɸÌ^ñ?d7b't†AGN4FGL J1254.5+2210¿ïO𺁊s@U@'(bõ™À9ÊôWÀ<UùK°Øz@¢v Ë@£iüóÜ?¶¢`<«¬í?¯«þöë"H?õUŒ·^¦@…Í»Š/C¿Î·_}>@¿æÕïUÑ¿Ùý"$½O¿Û…íÀ7h!¿çO;Ý%àd¿æp÷б^AGNbll3FGL J1254.5+2210TXS 1252+224?ïþ;Ð÷ºó?åÝH†Š?,Bðë«q»?åÝH†Š?ïõeAš?[Çìf8ÏÅ?Uý5rðè?[Çìf8ÏÅ?ïö¡3/Ç?PßÕ§E?R½™¾®'.?PßÕ§E?ïõ³ùõ­t?CðvY±Z?T˜ù(7'?CðvY±Z?ïýŽSæv?*‹¼½Ãӏ?3Ü'oòâ?*‹¼½Ãӏ?ïέáÀ­?½šå|ü•?x©q†à™Z?½šå|ü•?ïõ¡—u?eÿI²¶¬?UÞ¾/†Æz?eÿI²¶¬?ïçò×gIT?Xá™uwõ\?h
("ü?Xá™uwõ\AGN4FGL J1254.9-7141¿¦vÃTù¸…À!¥{"ÛœsÀ9û<š»ÉÀ<³"&jÎ@l·2[ÇÒ@>öÞN«?¿j%®(ó?Ã?áD‡@làÓêÎ@®qLÉ\U?ïòr®sEr¿ÜC¬ýúl¿è$dIU´¿å{ඎœæ¿êˆè""©¿ß'ÿùtöAGNbcuPKS 1251-71?ëåô/V³?ÔjJ'&Ƥ?Àh/B§‰5?ÔjJ'&Ƥ?ïïÓ6EL?q UÉ'×+?`,Éú™ëw?q UÉ'×+?ï€
ß#ˆé?HuU:Æ°?ýH%ï¹ó?HuU:Æ°?ïþ')÷?ðý$P?'ßOQ‰D6?ðý$P?ïìëåIy?bŠã—W?cøW/¦´?bŠã—W?ï£yíy?œÍÒÀ³?‡!¾[?œÍÒÀ³?î¯'}rq?›ï'%ïäæ?¥
ˆ-$j1?›ï'%ïäæ?ïú¼ðÇäí?5\½è*?E<N0!?5\½è*AGN4FGL J1254.9-4426¿Ú3Àá0@2lYtæ[êÀ:DN®¹¼OÀ<;hë{ä}@vîªíÿÍ@Uçþz¿?¼ýòÆ¿‰B
ø'´‰?ʎ"õ"@ƒái\æ?ïèÝ¿cW¾¿á	Ê^ˆv‡¿æ`Ÿ¨žð¿åqž½c£¿Ö5ÿ€Ô%Ý¿ïÿúVrÓ\AGNbll3FGL J1254.9-4423PKS 1252-441?ïúE®|ú?;—Ъž—å?FéGñÁµ?;—Ъž—å?ïëæ"^NÀ?kD©²~]w?dÝ}õP[?kD©²~]w?ïëW=å\?`ðã0R4?d¨ÂèۓÀ?`ðã0R4?ïøRÏR0?72}²©ÊZ?O¢µ}CÈ?72}²©ÊZ?ïóüð'5?P¯M¬Lvì?X+Làˆ?P¯M¬Lvì?ï"Ðà¾ØT?'ðä1¬ñ?ŠËÇ¿ß/?'ðä1¬ñ?ïÓ…ÿð?x~'|^ˆì?v{ö$òÄ&?x~'|^ˆì?ïÙàÜo?dò{Kê}ü?sÀv'S?dò{Kê}üAGN4FGL J1254.9+1138¿ÅŠ,Uë¼I@RŸ÷ÎÙ‡À9ýpƒöš&À<;á~4¹E@…6»©@õ–AöD•?¿Rj,d¸?ÊÐfŠM¡?ÿÀÑìÇ>@
©ØÎã¨[?ÙO³œz¿ã³ü†Î»º¿ëò…žeh¿è¹F¨Zý}¿à×Ë~3Ó¿ïÿœ,ñВAGNfsrqON 187?ïèo,Uý?'xò •
"?gÓg'«ª?'xò •
"?ïîÖɔ¢Ô?dªî‰=´?a)6FAd›?dªî‰=´?ï—mÒ7è?†)Þ	…ñ¹?Š$‹g·%D?†)Þ	…ñ¹?ïîS3€?L©¶­èI?a¬ÌlË?L©¶­èI?ïì_'O-Ã?cM5'?c }àìă?cM5'?ï¡d͛:?"Þÿ8áœ?‡¦Ì‹s?"Þÿ8áœ?Ëcãw?œÝGÑøF'?§÷óEvE›?œÝGÑøF'?ïdû'?…å4
'ú©?"l^…Ãå"?…å4
'ú©AGN4FGL J1256.1-5919¿×
ÀÒÇ@_0ÓÊÀ9Ç\ŸTÀ;Ï©mL3µ@ uxj…@újÊy5v?¸Í¡Þây¿™4YªÓ?â#Aî·Ù @B2<h;(¿ï¼IýzÂ?î—È©Q'¿æµLG×/&¿ÞyÀGƒL¿Ý€&Ö@¿ÞêiÀ¸íGAGNbcu3FGL J1256.1-5919PMN J1256-5919?ïú.ôxý?B¬Iw?GD.˜×Qó?B¬Iw?ïßúI»>?y¡ÍÔ	†)?pp'×Ù@?y¡ÍÔ	†)?ïåpF±a¯?nõ©¬`—'?j¹@ßáU?nõ©¬`—'?ïòMÕky?F 8ˆÔ'?[dV??F 8ˆÔ'?ïî%> F(?[8‡F¸?aÚÁD<÷«?[8‡F¸?îÇ{¤2œ,?®Åó{·¬?£ˆE¾Ž??®Åó{·¬?ïŸàÝ·"?ˆÖÝLä:?ˆþ>Cc€?ˆÖÝLä:?ï·Ëp"Ê'?v›o3ç¹?'
$ª7?v›o3ç¹AGN4FGL J1256.1-0547¿íðóô³›@Lˆ'ùD$À5…¼ÇœdÀ:}2ñÄÓÚ@"¿/üÈ@'d¼B;?y@X¿	?²Û''ãB@0­ÇGQÎ)@$ ?ö¶¿ËDYv=ôØ¿áVƶ2W¿å='AŽ@¿äsçŽ2׿é=Η¨(¿è·_èã«AGNFSRQ3FGL J1256.1-05473C 279?ïÍÏÂå1?'_éí>?ypge?'_éí>?î¤y¬ƒ?¶rÈ<¢Ñ.?¥¾d[ç`?¶rÈ<¢Ñ.?íë›\ÅÜK?¤Ú7ü?°£%O¨?¤Ú7ü?ïÛï_@O?ƒQÍî,
e?r{ˆW?"?ƒQÍî,
e?ïµí¥_u†?€CŠz$,?'"–´)@U?€CŠz$,?êÐ
#;æ­?ÐçI-y™?Ä¿×seJ?ÐçI-y™?ï^ÑPX÷­?•
ªŽ1?"%ÕîÒr?•
ªŽ1?íÿŸšïÒ?²nC…ûb?°‹(m?²nC…ûbAGN4FGL J1256.2-1146¿ïêO¦í{@IŠ<æÁÀ9r‹ò)ôÀ<øð@€-.â@§?þD
Öó—<?¯@ÄkTa×?›×Ù½˜sÌ?ì'Õ ™@cO•Gû¿ãèÔÀ6;{¿áKû¡K"©¿Ø}ŠDg
*¿à‹ã˜Á,†¿Ú…뜛¬™¿á¥sŒ¿–ƒAGNbll3FGL J1256.3-1146PMN J1256-1146?ïúä÷€?<j΍xR?G¼lÏôÔR?<j΍xR?ïò¼;Îù?Y£`9H"?Z‡‰Ó$>?Y£`9H"?ïÜØ}å?uŸû÷s?q"ö}p?uŸû÷s?ïæܵøõË?UÏjt/­8?i#J@Ã¥?UÏjt/­8?ïï¤öo ?S‹
…?`[	cˆ?S‹
…?ïÆ¢·á"k?'"îHüRá?|®¤×2p?'"îHüRá?ïÃcé£6?'Ýø"úÉ?~N2"}Ñ?'Ýø"úÉ?ﮬûÝB?vˆK…
í?"zT±'q£?vˆK…
íAGN4FGL J1257.2+3646¿ïRX¦EŠµ@TçÿX:TÀ9à?d‡À<gñBÍÚê@1ÆöI?þ¨™Fƒ?·›"™ÐK2?¹v´è)ŸŒ@Ìø×Òª@
ö8#¿çtØïð¾D¿×šƒT]Ð¿à¾V<"¿Ú«
š¸¨~¿æ~VG4qø¿ápq·Ó@"AGNbll3FGL J1256.9+3649RX J1257.3+3647?ïÿ¿M'?â0}"?hù¯.j?â0}"?ïõL‡ºkn?^ŲùP\9?Ufðë^4?^ŲùP\9?ï÷HP|?G¶øhö?QãÍ×Ó'è?G¶øhö?ïñjú''?DàG&ܟÈ?]*i…¼?DàG&ܟÈ?ïþb厠Ó?n!w‹£?)Ѧĕ¤\?n!w‹£?ïÝïd(–?sƒ¸%‡¹F?q(eIé?sƒ¸%‡¹F?ïó
O( ?dÓß*'c¼?YñëìO™?dÓß*'c¼?ïÔÅp¦Êô?bZwHJ—_?uG™\µö?bZwHJ—_AGN4FGL J1257.6+2413¿æTiõÎ4@U±Eà´áÀ;̀üê¡ÊÀ<Ûû()êµ@"1Žw&¨
?ùb¡ Ï?Ó¶…">C]?²Ýí§^Ô?àyt*tGÐ?û¢Ü)T?Î<©Ôz@8¿í¤u•®RŽ?ªá¡½våÝ¿Ú
÷À@wi¿zQ–åNË¿á\ǶãV|AGNbll1ES 1255+244?ïþ"_Ýz?ÎÛ}÷D?&Éÿ‹Þ·¨?ÎÛ}÷D?ïꂇÚ)'?u–]_ç?e}wãÝþ­?u–]_ç?ïñIç³5«?]™y¯?]l0ØÍz‰?]™y¯?ïùXLƒw?:QŽ-KÝå?JžÎž4ב?:QŽ-KÝå?ïþٔ±Rs?Úì>Yž~?"f³(Ú?Úì>Yž~?ï–
ÛÐB? vê'çk?Š}xÓZÃa? vê'çk?ïô'¨@?a¼øD#V?W°¯Ò?yO?a¼øD#V?ïÞá9–N¶?hPâⶬ?pcì(ò?hPâⶬAGN4FGL J1257.8+3228¿Ð'æ•Sll@UwîN&ÕÀ98dUêî À<	*	¾Å£@|%ÉX@À«;'?«Û¡&ŀ?ºS*tr×@µ›Á'@'ãçp'?ïÿîbHÊt¿áû–ä³s_¿äDÄU/¿äÚ
\ßÔç¿ê9yh¡ª	¿éN‰€Fâ=AGNfsrq3FGL J1258.1+3233ON 393?ïûÃÐ ®?5{{ƒæÈ?@ó½(~#þ?5{{ƒæÈ?ïõ=¿Ü¬ò?^ZÜDŽû0?U"€oák>?^ZÜDŽû0?ïÓ13à™?pw[ê?vgf8³I?pw[ê?ïüxË?+85`gÿ?<?Ñ¢Á:v?+85`gÿ?ïûsƒ°N<?@î£m'%?B1ñvMŒŸ?@î£m'%?ïÙ¨Fõ?z¡›WŸ">?s+Üݨž?z¡›WŸ">?ï^g‹CY`?'_€rD?"3µœ?'_€rD?ïø—'ƺÜ?@ú#Q+"?M£aŽg´ ?@ú#Q+"AGN4FGL J1258.3+6121¿ß.ã"ôÐ2@K߆
¢À;K›	bÀ<ò"Ì@"öàqšL?ýwœiW²n?ÇÉey¬iU?ÅÚyMBÔ?û$Éþ¼3"@§éÙM
Ð?í
z<@Œ?ìŽù,§'ø¿Èêû÷\ÃO¿Þêz\½p8¿äQÁÞÝ£¿åé÷ 54AGNbll3FGL J1258.0+6120NVSS J125820+612049?ïúÊËE?>0XØ?Dב ºM?>0XØ?ïܯÅø>¸?s&Hfe­‹?q¨q?s&Hfe­‹?ïë"f6?_ԙ=áßo?dݚ#Ôâ?_ԙ=áßo?ï(ùH€ÍE?|üö‰'g?šàÖöŏY?|üö‰'g?ïî·ó÷´?WÇ{ú%?aHÊs2?WÇ{ú%?ï¥L^í&?‰Ãâ#"[|?†¬èD¼6k?‰Ãâ#"[|?ïÇè´+b§?€Ãp	¬Áß?|¦+d}?€Ãp	¬Áß?íŽsI½}?¡"䌭Ú?³Œe±¦#í?¡"䌭ÚAGN4FGL J1258.6-1759¿ê4ÜÅW@FkÇÞP'ÏÀ97-Xþž×À;êU'þ@'°«@ݝ«w?°n²ÿàå!?Á–€JGÖ@I¬¤j®@[Ñsz¡?ã·íu?¿Ý`¥\E{4¿åµÔ}›6R¿äýÄy¿êéý)‹ê"¿ïÿùStAGNfsrq3FGL J1258.6-1800PKS B1256-177?ïõbsu?QºN™Ž?U;—‡ ?QºN™Ž?ïñvNT»ˆ?aPmù[?]cÉûπ?aPmù[?ï¬à
Fd"?€ñ³ «?"Çü¤:?€ñ³ «?ïü¢*6à<?&ž&9?:î­76ÛÂ?&ž&9?ïê,yä%7?b‡6öÐA"?eӅýž9†?b‡6öÐA"?ïÊ<þÒÈ(?{®N5/À?zဆËù?{®N5/À?ïMuº'?"Wv«ÐJR?–QN@¸¢?"Wv«ÐJR?ïögã"•?CK4$]â?S08ž)eÈ?CK4$]âAGN4FGL J1258.7-0452?¬‰›öpS2@LúRv‰ÊÀ:Úž´æÀ<_ãåî@!wãۇ$Í?ú—FBÐ?ÊRøur?Ìçø··;ì@Îå«Àä@‰þЪþ¿ãtyŸ(NÔ¿ïÿÉy[5±?ïÿç¬L#Å¿Öèq²Ë¿ÜŽòâ
K³¿Ý»u›AGNbllRBS 1194?ïýíÃ+R-?'x™…&äÔ?0'åΌì?'x™…&äÔ?ïï}ÄÚm¨?b@Pê|¾?`';6@Y?b@Pê|¾?ïç‡!-2y?mÀ‹M¶ú ?hxޒ4Þú?mÀ‹M¶ú ?ïî®"V…â?Pûáµ)©…?aQÝè²í7?Pûáµ)©…?ïþ‡"ü?!ϗGƒ£Ë?'ŽÜì¯È?!ϗGƒ£Ë?ï»Èg¯´?ˆ{ì…Zå'?
æ;¨à?ˆ{ì…Zå'?ïç"¤?T?r÷ᨚ÷?hÝã] "<?r÷ᨚ÷?ïÑYôèõ¢?r7v`öê?wSrÇþö?r7v`öêAGN4FGL J1258.7+5143?åÄríw+@PWÀÁü2À; ¼£‰ÝdÀ<¥~`X/l@1ˆ°h=+@懖ü?¼žWµs•¿·QԞ}Y?üÚÕٻș@ÚÉWLm?í}î¸u'¿ë¬dAÈø,¿è†çn2
¿Üë›D«¿ë/˜Ÿá²?ݘœä§´åAGNbcu3FGL J1258.7+5137NVSS J125825+514225?ïù/=§¢¾?A9O/æM¿?KCäá¨?A9O/æM¿?ïîÆ_}ò}?_7Bdé¤?a9 yÎsN?_7Bdé¤?ïÝT´.½¥?pܲüV|?qU¥÷¿ug?pܲüV|?ïÝyÛì­ñ?\Y!ù‰Í(?qCùÚÓr?\Y!ù‰Í(?ïëumÚô?a¬"øCnM?dŠ'±|ž?a¬"øCnM?ï–~Jøeœ?gOe0?Š`mHÅÑ?gOe0?ïÙ'	óã?|E^å+Óï?sl{ÍïŽ?|E^å+Óï?î{øI}M?—ˆöTx?¨NpxÔv;?—ˆöTxAGN4FGL J1258.8-2219¿ì³¬åH;%@DA¸d"À8ŒR7Û9À;‡Üßi‡ƒ@ÏZ/Kr@¦áÞ¬É!?¤h_ž¡?·î…?€¯¤@¶æS†Ò@ínοÁ!¿Ìl•?ì+¿â8ϟý¹¿åg­Ó
¿æZ§K39¿èꀥ+ô¿ëʶDËAGNfsrq3FGL J1258.7-2219PKS 1256-220?ïû¨>*¼?8j؄¿Ñ¸?Cé_Ãæé?8j؄¿Ñ¸?ïó-	V¢?[íw‹«†?Y¥í=Ç=?[íw‹«†?ïÛ¨µô̤?p¥µ`é]?r+¤è¼öK?p¥µ`é]?ïþß[<3.?Ÿ8•[w¬?"
NۀÔÝ?Ÿ8•[w¬?ï÷Š$¨ù*?J÷"UÝï?Pë·Àڃ?J÷"UÝï?ïË$nÒÏ#?} ÁàñV?zmÈ 7Vz?} ÁàñV?ïÌO[?¨?€ø"?Y|‰?yØ}Ì0à?€ø"?Y|‰?ïüZçÀ?2‡WEª?=+z7Œ[?2‡WEªAGN4FGL J1259.1-2311¿ì<-)ȧ@Cґ!%¶À9'u°ÐîÀ<
ìíԄQ@Ab…Ü#@Tò»sÞõ?¶‹4|?¥0â嬱?ëÝ[IŽ¿@O×X›Í¿ã‰è‹o4¿Ù£¤ÛA¿ã]'âïj¿ÚZ›WûQ¿å<á1ޟ¿Ø'·þ¯AGNbll3FGL J1259.0-2310PKS B1256-229?ïþ¨öó€°?p·tÏÝ?%p'e_ŸA?p·tÏÝ?ïó®Ioú?Z¶ï{²'¼?X£ýj[Ù?Z¶ï{²'¼?ïöý"FÌÌ?R¿öø\Ú	?Rق䈘?R¿öø\Ú	?ïÿˤP#?+sÇüõœ?æ'be?‹?+sÇüõœ?ïþ«N_ð?¯:¼jœ?%K°_iC?¯:¼jœ?ïÐ2ö€!?€\yëÍ?wæ"ÆÞ';?€\yëÍ?ïø»æ?[ƒ&i'À?M¿ñ<Û·þ?[ƒ&i'À?ïþ
¡u¨p?$ÁµÃ«Îž?/%ëH'¡4?$ÁµÃ«ÎžAGN4FGL J1259.5+2332¿êGª}[d@U~ªâ—9mÀ:ÎdÒ°,À<D(v@Îý@¯Ígý?@ÍDƒ½?ÄBðëe¿³t¬¾ÿœ?íä¦Þ%»?ÿ.¾+Ê3?¿â‰€Ç»–¿æØ^NêÊ¿èïæb.ï¿æûƒ¶¿éO}¶åû¿ïÿò~#¿AGNbcuNVSS J125936+233047?ï÷¸{±ý?`&Vìm?QôŽh6o?`&Vìm?M¡Y¾?"`k×gÑ
?ˆ"ì¡ød‹?"`k×gÑ
?ïz2?Ö°ž*é?®¶èèj?Ö°ž*é?ïÙ³1'–'?`é¡ÆÆà?s&g—®é?`é¡ÆÆà?ïêöÞÄÐ?jç:…Àò?e	ùî`øÁ?jç:…Àò?í!6 >é?ÂkåT5¿Þ?¶öJþ·'?ÂkåT5¿Þ?ïn&»?u?'Ž^SÒ£?';?e(uU?'Ž^SÒ£?í'ZÉ
†¨?«9ÕÓuw??¶Å)µóüÃ?«9ÕÓuw?AGN4FGL J1259.7-3223¿ïû;có@>r螺jÊÀ9{f¶~¢À;ðítA@èU³:Õi@–ªú-´?²=å~I‡?Àf0 .H¾@
Ä.béÚ$@µ¬]@¢Ý?ïû)ƒ£8¿Û—\¨wƒ¿æW!U;œ¿ä]sYN¿ét7	‰¿ïùûn Ç‹AGNbll3FGL J1259.5-3231LEDA 4075145?ïùv"Û·?Cþ«œ®
?J%°¼ìr?Cþ«œ®
?ïñr)y\I?`®Ó«KèH?]­ƒyþ9?`®Ó«KèH?ïÎäÂ6ñ¯?pÈÑq_?xž÷ÄøŽ?pÈÑq_?ïû»zónÖ?)éãh?_?A£s4?)éãh?_?ïé'4çE?c»|Aӄ?fØËX7Šj?c»|Aӄ?ïÈg
'tB?€ê£Ïö°?{Ìy3&VÚ?€ê£Ïö°?îöUbQ?•Æ2yÜ? š®¼r_å?•Æ2yÜ?ïòC×ù¯7?H×ùJÐhf?[xOï£}?H×ùJÐhfAGN4FGL J1259.8-3749¿ïûµâ
Ý»@9²c"úÎÀ9©N¬5}À<4\¬©@×@û6½\@΀ÌC:?²­¢ bl?sLù7üW?¿3ƒåþ!.@2Xª'
¯?ïé»ðÜvŽ¿àËXߕ&¿àߪõâoÌ¿á‹}w$$¿â፞¹"¿à®þúGAGNbll3FGL J1259.8-3749NVSS J125949-374856?ïýY«~.À?$ÿ¶?y?52¢%A ?$ÿ¶?y?ïôlXû?Z.ç(€˜:?W'Nÿ9­?Z.ç(€˜:?ïö 5T –?_6p£'ÛÐ?S¿•H4?_6p£'ÛÐ?ïø;ø¡p?=‡Ç=fåA?O¨eûÁ?=‡Ç=fåA?ïú›Ô©²c?<g[…P·¼?E­òz?<g[…P·¼?ïÑÒ`	ªú?x…ýێå?wÏúz—7?x…ýێå?ïóGØ(B?j_ŒW9ÁN?YpO9IZæ?j_ŒW9ÁN?ïñb¦eý?Pæ‹Z³ø?]:Äf<Æ?Pæ‹Z³øAGN4FGL J1300.0+1753?ȗaTò@T#ôörÀ:¶K̇,°À<|÷¤ëá@
º´2w@pÂàºÀ?ÃÆæþ¸?Ÿlp&궩?Ônw⏬±@›îÀèh	¿ì'+ˆDÀ?¢›+Ñ¿çØs>f6¿çE)Õ¼_—¿ïÊù=n˜?íýgŸKŠBAGNbllSDSS J130008.52+175538.0?ïí.¥œú?«Œá$r¦?bÑ[
À]á?«Œá$r¦?ïî5¤ks…?iG",.»?aÊ[kQ*í?iG",.»?ïql¡5g?~pLÞMU?ˆ£¤Éô6e?~pLÞMU?ïðЙyÒï?PlŠ3h?^^ÌÚßÃ?PlŠ3h?ïèJ	õˆi?kËyx	º?gµõõÙï?kËyx	º?ïYS¥»Þ?žL´D²åÛ?Œ)«p@i?žL´D²åÛ?ïNÀ\Hwµ?'ÊCÑ(?–'ôqɟZ?'ÊCÑ(?ï€K쒐?ƒF*¨Ài?ú­*/ø?ƒF*¨ÀiAGN4FGL J1300.4+1416?ºLy•Ã Q@S>iƒQYÀ9tùòŸÅ-À<<Šk(m@_öèª"ÿ@†dÆS6?±—"–}/?µÝ';¦t?ûÌO~ÃT~@j«²¿ËÜNõÜeœ¿æ£¬!Üs´¿êHõ!¬‰¿åòI(gþ¿èò%ìù'þ¿ïü±®¤AGNfsrq3FGL J1300.2+1416OW 197?ïüÑŸ?:ÛÛñ´y?9qÓDƒIÖ?:ÛÛñ´y?ïòzå_¦ë?cN/y®?[
5Áãy´?cN/y®?ïÕRՏéí?tçxûa†=?uV•N¸u)?tçxûa†=?ïïp¯PÌ2?PaéŒëÀa?`P›õþ˜?PaéŒëÀa?ïùq©n+Š?D³'Pá¥]?J9Y6N¢?D³'Pá¥]?ï½\§ÿ@›?çhا?€¨Õ÷@ÝL?çhا?ï²µ[/ëD?'ÑY¼na±?ƒR©)o?'ÑY¼na±?ïœ@b›«˜?€~ÛS«?ˆïç_ôR?€~ÛS«AGN4FGL J1301.5+4413¿ëx;DÆûÊ@R1×Ûô‡ýÀ;Q3Ï:eÀ<×ÊZ+Ł@4ºuÝ&â@i[»èxû?™ڇ™x¿ˆ»Ö
ù3?ǵ­áÐ*@/xº{çW¿ë‹hH¾µ³?濞`¨·D¿ç£õ¾¸¿×|ÅW7Ÿ¿èŸÐ_©]Ý¿Å[¿XðÜ÷AGNbllGB6 J1301+4416?ïþÄ|Nã›?jë3Ô¿?#¸?7çH?jë3Ô¿?ï÷šôÁ4?T2և"Å×?PÊÓè%?T2և"Å×?ï餅Ÿ«p?q?ƒªmG?f[z†Ð/€?q?ƒªmG?ïú²8KöÎ?."]Ÿì~?E7…¬+?."]Ÿì~?ïü¬­é%?5Åäaœ
?:š–Ï=B'?5Åäaœ
?ï܀K¿Ç?t,Œ
´…n?q¿Ú>Yé?t,Œ
´…n?ïÖ7ÖAPé?~úû(ÀÁŽ?tä×ÈgY?~úû(ÀÁŽ?ïí$PõÄp?TVBa0•?bÛ®Ô¡§å?TVBa0•AGN4FGL J1301.6+4056¿Òq¤¡+@Siì,äeÀ;*@tdVÀ<Ö=Jä*@ &H½´"?ý
‡¶B?Èr_™ãA?½N䔔¢?õ")'°I	@µáL‹žÚ?¸f§>r×c?îŽCû"¿ÈydDùb¿áR"!7]9¿æ½+o"O?±Ô¼ZcαAGNbllRX J1301.7+4056?ïÿLàÈ&?«kÍî?cääì¢0?«kÍî?ïô(¡3ìÂ?[:÷3eû?W®½'§ô?[:÷3eû?ïöëcˆ2?B=ÐThȜ?R)8ٞk?B=ÐThȜ?ïÞ ®…m?VY
¢W?pïó0Lm©?VY
¢W?ïþò%™9?sÎ>»? ݪŸ…r?sÎ>»?ïÙmpµŽ‡?wHßß?h?sIG»6<Ÿ?wHßß?h?ïó	ùd@®?f¸e©&{Q?Yì
`¹ôÆ?f¸e©&{Q?ž°ý?v¡D•Ô'?ˆ\˜W0Z¿?v¡D•Ô'AGN4FGL J1301.6+3336¿ÝœÏ¢Ó~@TÉØ­«ŸVÀ:z/w¼ÐÀ<t[íf H@êÑ;F}@cH9Tµd?ÏAQ'Ó?®…-âønw?æ}+Ç.'@ä-̖ñô¿çºÂ^3çä¿ã1¹€¿®¿æšýqÛ:¿èO–áXu¿ïûãp}@¿ï´ÉÀþ¸WAGNfsrq3FGL J1301.5+3333MG2 J130126+3337?ïýóQàŒ6?$zN±Y÷?0eo¡E°ô?$zN±Y÷?ï÷Á°JF?U=âã1a¦?Pä|Öe2ý?U=âã1a¦?ïêu͕'M?d¿ûãýŸ4?eŠ2H|›‡?d¿ûãýŸ4?ïðy%õvÔ?K!à2h¢?_
´(P($?K!à2h¢?ïý›™?/KaÃÛ¬ó?3#6醣ì?/KaÃÛ¬ó?ïÚ䯀a?y"?jRžþ?r¨_?€?y"?jRžþ?ïïD×r?i=ÿVB(?`»ã­NVI?i=ÿVB(?ï¹¥UÓ?s "Çßã?»–µß"?s "ÇßãAGN4FGL J1302.3+6901¿ßÌG€G8@H:}ªOÊÀ:ëè&Åf§À<ʞc,ö@bdþ²M@›?{@?ÅM%ã‹"?¡ðþ…V—?ÔhöÎþÖ4@UÞÂî| ?î²k!·	í¿çM³9ä'¿è-ê¿îI
{^¿ÊϵŠeõ¿ïþ2Àœ'ÈAGNbcuTXS 1300+693?ïþˆò‹?"ÓŇÐ#?'pӚˆ½?"ÓŇÐ#?ï÷ÓӞ›?R‡?ÚÍtÊ?QÐX|~ºË?R‡?ÚÍtÊ?ïÖPÖԄô?ylóÜзÓ?tה‡O)à?ylóÜзÓ?ïú>)M?74ú©¼6&?GŸIž?74ú©¼6&?ïþoeØ:Ù?.D³‹Ú‡?)	¢Ø®X
?.D³‹Ú‡?ïÙ~86Ÿœ?s	ñMø?s@ãâ n)?s	ñMø?ïЗ‡$è?{U9àyçr?w´<qn,?{U9àyçr?ïÑ\'Ñš×?nj> V?wQ¾xöÚ?nj> VAGN4FGL J1302.7+4750¿Ë™]‹Ãºw@QJS5À:ûâTôNÀ<¿cí@»õÊd@Xb—¤Í?Ä|`8Nû翶µ_©D?ðùV̕o@'âý:Ó»?¨gmޑª¿ìˊw½¦¿¿ç§{9\B ¿áÁCâWùf¿Û!²Ø/Ÿ¿ïÿÅbu@AGNbllTXS 1300+481?ïûè&M$T?DÝÝ~"^?@_f1€2B?DÝÝ~"^?ïàEÜ>k?'¬ïpý?oº#ùî'Ã?'¬ïpý?ï·$ȝy^?gLl3?'6Íᐤa?gLl3?ïë;aCֈ?S{ºæçDc?dвŠ¼?S{ºæçDc?ïúq›×??N%¦¼ýû?F9ÒDm?N%¦¼ýû?ï85¨"?¤NÈ®ËÉ?˜þP'™?¤NÈ®ËÉ?ïªsßà›?…/@| N9?…c4˜=B?…/@| N9?îˆúDK«Ç? ("":?§p[¼!*ˆ? ("":AGN4FGL J1302.8+5748?êîŽŠê ½@MŸ©\…<À:W8õêÓHÀ<¾r¡L%@ÐÎý'@Y?¼®q˜?´B®Ñ9C¿5¶p?I?åÃ"ÿßHÐ@sã*\J?bmˆo¿è=þ"Ci¿àöÝâžÆ)¿âEbk¯ü¿âe!«ÌL¿ïÿÒþÀùAGNbll3FGL J1302.6+5748TXS 1300+580?ïòJ	6¤?'h—5?[jái¡¸,?'h—5?ï÷Õ22={?Q¼U™'"%?PU›Œ cw?Q¼U™'"%?ïéåޅuº?r³ÅÓS
©?f!~©Íõ?r³ÅÓS
©?ïùfïß\®?4À m¬€?JdA¼é?4À m¬€?ïúß9wv??ìƒÝR²?DƒámÍ5??ìƒÝR²?ïÞéPLYÜ?sqh~í¼t?p‹W¼Fn,?sqh~í¼t?ïàQýS/?~
FÒu&?o®c/ðÌ?~
FÒu&?ïñÝ Y§;?HlÆ=uõ?\D¿]/©d?HlÆ=uõAGN4FGL J1303.0+2434¿ëy¶\·«@U–Å—Ne¿À8Ì£Ho›À;ÃÀ…–­V@u¸"Ú¾@‡5ÜZßJ?¨ÎƒKŠ©?´Ýv=I¸@¦˜5‹'@ÎØÈ-¬?Óe±ÀVò«¿Ú¡Q¿tè¿â™ÀGƒL¿âUŽU™¿æ@&Ì£¥¿ëÐøÀñwQAGNbll3FGL J1303.0+2435MG2 J130304+2434?îà7Ê`z®?ÆÓÉz«u?¡üƒ[°# ?ÆÓÉz«u?ïò1ì':?g%TÎ8ˆ?[œäœ|?g%TÎ8ˆ?ïÝtGOŸÐ?s0ò™ø?qEÜw" ?s0ò™ø?ïýoºÖˆÁ?#rPC™‰?4''?Bh–?#rPC™‰?ïý•ùÀºŠ?2¼ø'õE?3P1¥' '?2¼ø'õE?ï¦O鈀~? A7J˜?†l¨.´~? A7J˜?ïÝiFâßÖ?yµÕ?0›?qK\™ŽÔë?yµÕ?0›?ïúyXäü!?78H=Î?Fœµ-'R?78H=ÎAGN4FGL J1303.6-4622¿ít£–6}@0s§ü2ëæÀ:±®£íÀ<AÓë¤ÿ(@¹èÁÊæ@¿@D"­Ç?¿—ç'ËÊ?Æ"ïĦ¯@ˆì9ò@fš%Ç:?ïôÁPlÕ?Ïv<È2^L¿ß—dqē¿åˆabñfà¿è×a {{¿äoØ ?¦AGNfsrq3FGL J1303.7-4619PMN J1303-4621?ïïñÇztÞ?^!oJíbd?`8"+Jh?^!oJíbd?ïävÑü?t}R*í?kàŠÜ/?t}R*í?ï»îLh'K?zªtWV?lã6}a?zªtWV?ïó‡ÓJ?@É-ãŸHK?XðXåkÌy?@É-ãŸHK?ï°¬Q}l?Q20–?ƒÔëůxÞ?Q20–?ïMmwçE? ÑðÂ@
?–RQ	­g? ÑðÂ@
?îOä*¦6?¡_ ~©?«ÀÅ8¡?¡_ ~©?ïÚþsì<?^v`šÏ˜'?r€Æ,«Iç?^v`šÏ˜'AGN4FGL J1304.0-5539¿ïÿ%¾;˙@´Ì?ß À9ésÉ%x`À;‹)ƒ‡@äŒu™µ@1;â.^?¼a™¢þÈ¿§ïС²[¡?ç2t[òo@›yòŠKž¿¼Ÿa.Ä
¶¿ãk›ŸXJo¿ëÐOt…
¿ÝC =͕õ¿ïþ"þ?ïâ
;Qå¦AGNbcu3FGL J1304.3-5535PMN J1303-5540?ïëҟRHÖ?`€Ñ &à?d-`ÜqÚ?`€Ñ &à?ïÛ=éD§¥?}Úf&ÉB'?ra]¬-›?}Úf&ÉB'?ï HýAV.?ƒÞ£÷Zà?‡íÀ¡ì"?ƒÞ£÷Zà?ïølê¨ÄŸ?;7¿
i e?NLT÷ÅÒò?;7¿
i e?ï(†è·ë?›u¶1ø?šï#¨:£?›u¶1ø?î­lÙ-i?±¥\¨±ìJ?¥)2lM€ó?±¥\¨±ìJ?îyã×P?ŸyN/•?¨aÏÅ"ÿ÷?ŸyN/•?阮Vƶ2?{m­³ÿ	Ú?†jGs;t?{m­³ÿ	ÚAGN4FGL J1304.0+3704¿ÖÉN1±@SíKƧïžÀ:ÚñfàêÀ<žÈ:£j@Á›÷—ј@;^ʐ²?ÆcÄÄ?±h^ÊKú?æ¢6Æeª@¹©ñb?ïûùá
÷¿à™Ò¤}"¿çڄßÄK¿á¦W¸M¹Ç¿ëKz‡…šß¿ïØODù"AGNbllWISE J130407.31+370908.1?ïü½–V¡«?OeҊ‹Bs?:M'Q¿?OeҊ‹Bs?ïöG‡©A?WMþqyY?Spñ4®.?WMþqyY?ïÆâ$?»¦7ûW™?|Ž÷fjÎn?»¦7ûW™?ïç'>—¦Œ?P)§È"?hmÁ¨ò&?P)§È"?ïü¼ýìÕ?4ÐÙÅ<öí?:ªX)?4ÐÙÅ<öí?ïڐGº™?véh_͏?r·÷£?véh_͏?ïÍ÷sƒI:?¥@Ùze?yFLÒó?¥@Ùze?ï¤á¾õQ?rhN¸¿¸‰?†Ç¿ÐB«ª?rhN¸¿¸‰AGN4FGL J1304.2-2412?ÖÀ¼?®8@CH×ðí=†À9Ëúú݁PÀ<(ÒO̲@÷õÄè5?þNŕ æ•?¸òƱ¿S?°­Ù'è‹?÷OÙý6÷ä?ÿA‰BŽ?ë\|m8è¿Û¸¬Cë<O¿âkb^ÄÜh¿Ø6%€íü¿àk'³ò
t¿á¶}euüAGNbll3FGL J1304.2-2411PMN J1304-2412?ïù"˜R¿?@›ÓiT*?Kuž:kYþ?@›ÓiT*?ïÞ ýĚ?pûcÒC?p¯7 _?pûcÒC?ïäJC‰ÜQ?lQ/ÎN?kµ¼ÿ&¶?lQ/ÎN?é5¹?n»ÒäöÞ?ŠÒE¯")?n»ÒäöÞ?ïíC°Œ'ã?Xg‰z]VW?b¼O­6Œ^?Xg‰z]VW?²Ý§)?JwËÓ"ˆ?QSVT¥"?JwËÓ"ˆ?ïÙ³y?{Ü¥¬¨7=?srõ&iú?{Ü¥¬¨7=?î;^bX²?"Ò³Ù›C;?¬J8"¦á?"Ò³Ù›C;AGN4FGL J1304.3-4353¿éY¾/ٕ@2êœo6ðÀ8zËïW;PÀ;wg)ÚÄÝ@E3'¹XQ?ûÎU}àÖo?¥Ø‰n~7é?¸Lݾ·‹G@ÅO±@|÷xÇçá?ïéXÎG ¿àùoߌ¿Õf¸Ü*ï¿Ú
ƒ÷ÿ¿àƒákÀB{¿Ý_ò.+AGNbll3FGL J1304.3-43531RXS J130421.2-435308?ïü£È$O?6áå×Þݺ?:á¾£@èó?6áå×Þݺ?ïÕOÏîa¿?‡Èž˜E¬i?uX|Œ3?‡Èž˜E¬i?ïÅ`K3þ?€g'(ºb€?}OÚZÂTâ?€g'(ºb€?ïö7ÚÔ¢?<@<¾`2"?S'èÀ‰Jª?<@<¾`2"?ïþõ£þ?*lñ%þþ?/¿Clöà?*lñ%þþ?ï
CÄÚ?­Ÿ";Ï¿?žN"
è·?­Ÿ";Ï¿?ïÍ]nM?ƒHgçá¡S?yQ?cÉMC?ƒHgçá¡S?ïç(£ëµ¤?Vü>ÖÄ>?h×[ô­ôh?Vü>ÖÄ>AGN4FGL J1304.6-0348?»žjÜ—#@MrK èBtÀ;g€t.¦À<¥Ó`dĦ@?d3?ýùÓ`dĦ?×@.C_PH?ß× ìt2?ýŽ0"óA¬@	/^Ä;¿é«æ¾š¨¿ìì©@։å?ýz¿ŽËµ¿æI;þ]éj¿äþø™q¥¿ïÿYFÃ2ðAGNfsrq3FGL J1304.8-0338PKS 1302-035?ïþkӍ±.?#'eÜK?)BÆÆ^F<?#'eÜK?ïñ4xáë?b'¡j6?]—
î:8?b'¡j6?ï¨/LÚàG?|A†Ñ¡ü?…ô,»‰~P?|A†Ñ¡ü?ïõbÍՋb?@°§û'—?U:dpfG?@°§û'—?ïþ(Pšæå?*£úŒ?-z÷±i§^?*£úŒ?ïÃÊrÝöž?ƒ(¶Þž
v?~ƕÔ$É?ƒ(¶Þž
v?ïš<(3R?ˆÏ''t?‰pöñ›W?ˆÏ''t?ïÚæ£ìŠ?dP¤ÙÞ×?rŒ­óü»?dP¤ÙÞ×AGN4FGL J1304.9-2107?ç™çÕR@Dл¡+^SÀ:bßÔçM'À<>-o|@š,œì	~@2ç-¡"û?Ä_DB™®?µÏžcWé ?ï'ø!dS½?õ¿Ý5¥©?î.Iq?栚tŠìX¿æ:)Çy§¿ã"9°ûµî¿à‡Ý~›<¿ïûï< AGNbcu3FGL J1304.9-2109PKS B1302-208?ïïê>UY?aV°¿ï"?`ÿ¨íwM?aV°¿ï"?ï-_é8'?¡àð¦]ܱ?šTÒ…>?¡àð¦]ܱ?ïÏTڀr4?wÜwæ3ÿ?xU'µx"?wÜwæ3ÿ?îªÑYƽ?É´	IG?¥^bçÏß0?É´	IG?ïáÓ9/?i¸«ÉÐ?nè,¯¢xÈ?i¸«ÉÐ?ì͔1ó¢?Àã¨.ev°?¹"^pÕ~m?Àã¨.ev°?+ć?…ÍdШÇ?‡S5,ðÑ?…ÍdШÇ?èæ½¥M¾
?³Ý‡'ôD>?Ìe	jÉ×?³Ý‡'ôD>AGN4FGL J1305.3+5118¿Â5•iš^¢@PkM:'£À:îòüÀ<Å'o(­@1æ×æ@;Ù_'F—?Òü4g??Ý_+ÿ¸1Š?úY
wt¬@ò!°~ã`¿ïûUá³äž?ïcóÅ_¿ìoC"º"¿ê§Š$Ô¿á¤jB"ùG¿ïÿ³ÿÌS€AGNnlsy1IERS B1303+515?ïö†¨ñ€?s'u§c¿?Rò°xŽ ,?s'u§c¿?ïß¿µ&ß?ƒ	b ©n?p %vžx??ƒ	b ©n?îúfÜêŠ?'`9ÎV'? Y'3òì^?'`9ÎV'?ﺤ¯Þe¸?mµ×zÁ5l?VÔ>?mµ×zÁ5l?ïõüÃX?b9ý/Ë´œ?UÌŸ@€ƒ?b9ý/Ë´œ?ïm¨S_'Q? +òK\Uß?'Jõ‹v¯ù? +òK\Uß?íõùŒ…!? SɄ,šÊ?°P3ž7ïù? SɄ,šÊ?í;(¤u&?§*žÀô4?¶'Æ»¸=Ï?§*žÀô4AGN4FGL J1305.6+7853¿ì©Q§´Ü¸@CÿyÈCÀ:EFmCÐÀ<¯:ঞ@Œè0Uˆ@ðàpÀ?¸­G`ç¡d¿I]ÏÖüØW?¢Èè!ù
T@­˜¤§Ö?ï]=Þ1ùø¿â²ªפ—¿ä'›…,$K¿à;ú'½˜¿ç»üšð±®¿ãÑqw; ÀAGNbll3FGL J1305.5+7854S5 1304+79?ïùÑÈèš;?:§pû"?H¸ÛÊÎ)»?:§pû"?ïõ«Lìº?SŠé>þ±Œ?T©eÔ!˜?SŠé>þ±Œ?ïíòl¬õ?^LKßÒÆ?b
"°YK6?^LKßÒÆ?ï¾0ð7àí?jHÐðp0?€sÃâé|Ú?jHÐðp0?ïé <ta?`´¨ü~T?f_ïê??`´¨ü~T?ïÕC•ùHx?t¾k\ã?u^5zÐ?t¾k\ã?ï×÷)[‡Õ?~*,™§«?tkA½õ¤?~*,™§«?ï55S@fD?†N÷¢rd?™YU™«~?†N÷¢rdAGN4FGL J1305.9+3858¿í=s,aK¹@Sq€ˆP›úÀ;"Á¯bX»À<ópˆÿ£@™¶¯T@·
è`Ý?ÍSÄ[d*?³G`ÖsY?å)¦¢@²"@ÖAj®u?ïúÀ~gå¿è™K`P¢°¿Ò¦…eZ!ß¿è17æ Zé¿ì;yÞhUª?âɛ?-±AGNbll2MASS J13053124+3855218?ïùö1†F?J"9Kú[¸?H':IO¾ø?J"9Kú[¸?ïöMç¿lg?Wa·òtx	?Sd0uBŸ?Wa·òtx	?ïxTfö‡?ŠvKœm?õs>xý?ŠvKœm?ïäüˆÉŠ?S¢Ñ¼KÑ_?kw=U`?S¢Ñ¼KÑ_?ïúY ¸ÐI?CRÒ,‰Zð?F™}k8?CRÒ,‰Zð?ïÙ*Nï7—?x+°]¯vc?sjؔào?x+°]¯vc?ï•Nr÷ä?‰¦Ôwx£?Š¬cOúvü?‰¦Ôwx£?ï2QÙ3?x4è¥Ì?Œ3kdk
?x4è¥ÌAGN4FGL J1306.3+1113¿Øc­xb@RmÛ"Ðå`À;1Óºý—À<£Êz5˜@ }¹!]¹?ÿÀëíúCþ?ÅџÅW¸y¿l‹.|'3o?¤ëÜ1™«@Jc]¿ïÿý±q&´?ïÿáÍì¿Ý ÎâP¿àÅ%ƺd¿ïïícEI¶?ïYà37AGNrdgTXS 1303+114?ïõ´6š?Q'ËH7,4?T—çóٓ?Q'ËH7,4?ïñ.Flÿe?b¿ÆÖõäÙ?]£r­õö?b¿ÆÖõäÙ?îý²T?a.?•³Í2´n? $Ú·¾j+?•³Í2´n?ïï^Üs!Ï?Q%Úî˜5?`¡#°š W?Q%Úî˜5?ïòÁ"›",?ZñYJÔLŽ?Z|Ös¡XÇ?ZñYJÔLŽ?sX"Gð?Œ²q]¹E?€›)â]Ÿò?Œ²q]¹E?ï=ýفˆx?"×˶¶Ü?˜@DÖ®(ñ?"×˶¶Ü?ï´çt)-Ý?zùØVÂQB?'Æ#»*´?zùØVÂQBAGN4FGL J1306.7-2148?ï1¤"'.Ê@DuöM½ùÀ9ó~°à<À<,YÜë(@s{ϯ*P?ÿ³!Dô%×?ÂGFe•5?ÉL²`9ü{@¶n¡žJÙ@ ZÑ1áO?ïþá77¥¿çšf³"?ã¿Ðƒp!ûþ>¿á†UºF¸K¿éi¿·:"Q¿á^˂Iñ¼AGNrdg3FGL J1306.8-2146PKS 1304-215?ïwS@^?µÈÌCšFƒ?ÑfîT?µÈÌCšFƒ?ïÃaì¯W?€QÀ×?~O	Áâps?€QÀ×?ïRÁK—á'?'uª'õ?•§ÖsiÕ?'uª'õ?ï0e(\?"•ÎÿÇ?™óZøkƒ~?"•ÎÿÇ?꤬ðìð6?ÀÌ{÷¥Ç?ÅmL<L?&?ÀÌ{÷¥Ç?ï_~³œ?—‹è0I¦?"=«UZ…?—‹è0I¦?éÄߚ§-"?²«<Ihq?È쁕cKv?²«<Ihq?ì")iþë? é="¾?»^´°@ª? é="¾AGN4FGL J1307.6-4259¿Ìºð÷ys´@3ÇÅ£ãŸÀ8¦17°pvÀ;¼-Qqâ›@Y24…˜±?þvbBw†?¤­r¿e00?žN%ûÎ?ö˜l¨ŸÆÚ@	É~8À¿ØàᬭȿÍc)Å÷¿Þ$_۲ĿܯD3‹ž¿àÛçQ³Pû¿ÔcÛÝrAGNbll3FGL J1307.6-43001RXS J130737.8-425940?ïþy-ςE?ÌÌà•¢?(m$;¸®®?ÌÌà•¢?ïì}£ˆŸ?dæüPV…?c'\ƒ¿×?dæüPV…?ïà›/_­Ô?{l–>åÕÈ?odÐn×Ëò?{l–>åÕÈ?ïîÍEm?RÞw^ü"Ç?aâ2û+
??RÞw^ü"Ç?ïú§4%»?:ÀüEéª?E‰bcswQ?:ÀüEéª?ï‡iØÙÿ?žeK´3xÓ?Ž%‰Ô	?žeK´3xÓ?ïæmz	?y±ÕÄÒáD?iô'b:4?y±ÕÄÒáD?ïԃ$(?mûZu2¯D?u¾m¸¼í?mûZu2¯DAGN4FGL J1308.4-6706¿ï©LÎÿpÓÀ*"'AÀ9!'ˆŸÀ;™)†âñ@ J5Ù*Ô@½¾hê?´uÞÝp‰?¹YÝìÚ´A@ÿ}>@C@ké?Ÿ'?îçuû.ßç¿ÓЕ"60¿ä¬j¹¦¿æ:"`R%<¿äXÞ=¿ïÿÿ" 5•AGNbcu3FGL J1308.1-6707PKS 1304-668?ïþà_Œê?#öÙnދ?/qöZÑï?#öÙnދ?ïæÃ
"»
?€6im´½Ò?i<õádz¦?€6im´½Ò?ïÖóêükT?x[*s+?t†
º'9?x[*s+?ïý
lz&¸?#/çñ|,+?7"šÛ
~K?#/çñ|,+?ïüÀ7	£å?6övîa±?9þHhL69?6övîa±?ï<H©ÇÛ?¬Wî܊?˜vêÛ6¨?¬Wî܊?ï©ÁŽ™û?…GAV8P?…œO2kƒ?…GAV8P?ï÷YÁoÿö?C9ç¦Æ"?QL}ô~?C9ç¦Æ"AGN4FGL J1308.5+3547?è©+'ԍê@T&»ó¡MÀ9ëÂÐʈOÀ<f½Ž©|@j°†5á@tÌ?ß ?µóÁI5ÿ?Í[‰ûkò@¯ÿCAž@Z3k	?ïnÙgÒ¿ÚÊZ+ŀ¨¿ã¼œ2Ñ
¤¿çGÏ[¦¿ëä¡ÿ¿ïÑ ;tJAGNfsrq3FGL J1308.7+35455C 12.291?ïRžtùt?¶Pú7äÔÉ?•¬=j™—?¶Pú7äÔÉ?ïå®À>•?ƒ?|¹WX»?jQ?mÀ+6?ƒ?|¹WX»?íŽSù¸yj?¢R1Kã"v?³`1ÎA2?¢R1Kã"v?ïÓIqÊ-ò?`hSí85O?v[G9ã?`hSí85O?îØîW"?›À#Sé¢?¢ :Û?›À#Sé¢?ïÃÂô$Æ?'ò¢'ó'w?~…Øð½/?'ò¢'ó'w?èõY͕Ž?±"<õ^#g?Ïô*˜É©Æ?±"<õ^#g?ï@õ—àö"?ƒƒkÄ¢?—áM)_|?ƒƒkÄ¢AGN4FGL J1309.4+4305¿Ôù!†"áH@RhVWûi˜À8êé—îâÀ;ʟGX"&@ðÀΑÈë?üMJ†6‡?§xæàcr?µb»¶úÓp@_$•á~5@aÁŸÈê?ïêv–_Rv¿ØHŒ¡8ŸY¿×4B<e‹ö¿Û}»ÂŽZv¿âÖùvy!¿âçrj€§ZAGNbll3FGL J1309.3+4304B3 1307+433?ïüt<4[?4gTý'?<^¿¼yú?4gTý'?ïÍ+_‡Ø…?Œ_›ƒð=?yjP&=Ò?Œ_›ƒð=?ïÛ¶ãxØ?t"Ĕ
Ð?rv$mGT?t"Ĕ
Ð?ïRŒ6jÜ?yƒl(?•¾Ž~Zn?yƒl(?ïø'*ޝQ?JÑ8mƒ)!?OcTmZH@?JÑ8mƒ)!?ïbùÌjc?œ^#í]?" ÌDºå²?œ^#í]?ïÆÉ)C	.?"Ñt²Î?|›kw8˜è?"Ñt²Î?í"|2øÈ ?œrJáÖ2?³Üj_€?œrJáÖ2AGN4FGL J1309.6+3718¿îwÅ~@SÇiÂ;ySÀ;¿B$g¾UÀ<õ²6ci@!Cš
,Õ?ýåù×ÇÓ?ÅxÀƄ3V¿¨ŽïÇx¥?äòÂàdÚ?üê#!BE?ð?àØ ÀaŠ¿ÃSGOÊÄ¿çñ-Õ%`ã¿á…\–$?Ä?ՂþÍ{AGNbcuFIRST J130948.8+371651?ïý¾"#c?*?妝Íà?2Ýàˆ]?*?妝Íà?ïç2@ïßK?q$7N??h;ÒG¼Ö?q$7N??ïÒø×(¶?xøëÞ¢³?vƒ"sŽÈÓ?xøëÞ¢³?ï©èý–*?mí/^`Š9?…½¶K¡¬?mí/^`Š9?ïýRÿ´ß#?2[Dø?5h˜Ìu?2[Dø?zðÙi?•î»|EàZ?‰ÞáQˆµ?•î»|EàZ?ï½#ïÉQ?ƒ,‹ãqS¨?€·U=?ƒ,‹ãqS¨?îró‡‡Ú?™È5ÌÀÝ?¨ÞPÅÏ´\?™È5ÌÀÝAGN4FGL J1309.7+1153?ä­ýJ²Å~@R‹">iƒÀ9ÉQì[ÞMÀ<J@~uPå@-Øjå§@%ð|Õ=µ?µ ÏXmTl?¯S"'Û9?÷–…³2ÇÓ?ÿÄ¢–?è*·c®ü¿¬À=àÇg¿ãshãh­¿á'­Ãó	¿ç¥¹Þ²§¿ên¹PïÝAGNbll3FGL J1309.5+11544C +12.46?ïö©'M3©?IÀL[?R¬Ýœ'm7?IÀL[?ïzé}ä?Šq¼
•r?¢ÞìÓá?Šq¼
•r?ïÅÀþQC?|þN†Âº?}€»ážê?|þN†Âº?î¯å°ôT%?úÕX`?¥¤ïÞÖ­?úÕX`?ïÓ¬aÿœ?nê£À@¤Ä?v)¸Q¿â?nê£À@¤Ä?î_k¦(|?´® †<­v?ª	NÑQõI?´® †<­v?ïnA‰2?'OË®åg@?'7ÎÇz‡Ã?'OË®åg@?ê…&êiY¥?°ý	Å?~Š?ÅëdVZ™m?°ý	Å?~ŠAGN4FGL J1310.2-1158¿æ/š½¹'@IPØ]ú‡À:KÏknÀ<UBí»YÞ@ˆ_X@$(ƒ¬ÈK?¶þ"n\T?'¦Ø؄ø?Ýô^´kW?þ&'Ë¢¿ï(,ÚSž
?åzVs'¿âœ°ožôL¿ãdT"—½¿Þ¤‰ôaf¿Ó°
ĎºÃAGNbll3FGL J1310.2-1159TXS 1307-117?ïù¼ªæí??¿"µ?I
WÒS/"??¿"µ?ïìÌބI?do­Ú:Àé?c3!QÄ?do­Ú:Àé?ï܃%[P«?r…¤ò?q¾mGXêŠ?r…¤ò?ïÜÇ[FÛ?[1ïⶤ?qœRUÀ*m?[1ïⶤ?ïç¶$¿§ö?c~ex
@á?hIÛ>Â)?c~ex
@á?ï£.˜Ä²w?—5h‰Úž?‡4YËcÆB?—5h‰Úž?ïÃñidG¨?fç|'?~K.?Ä?fç|'?ï]Ú}ÜÇ
?"ðâT@?"D°FìV?"ðâT@AGN4FGL J1310.5+3221¿äô  ã@TÕ=1¹¶pÀ8M_ŠªŽÀ;[ß-ø`Ï@³±_^	v@eÊål?¤6NàQ¨®?«DTÚ<L@`ù£v'@LVjoàc?ï%tc+Y¿ãE& RÆK¿äe·]®1¿äF'ÌÍ£Œ¿ç™!ú{²¿éécÜHkAGNfsrq3FGL J1310.6+3222OP 313?ïý6§[ùü?);b'?6JÄø}?);b'?ïõj.‹Èd?Xøu†
¹Ì?U+¢û­÷?Xøu†
¹Ì?鸞Z Vï?‹26K%F?†×éb9?‹26K%F?ïô¢ÀE<?K7".LVõ?Vº~ñî‰|?K7".LVõ?ïùš¼•ƒF?E^R%XˆA?I•
]ˆf‰?E^R%XˆA?ïÞPÆt¡›?|u˜È¸9ô?pל¤²òœ?|u˜È¸9ô?ïk"mÂ?'ßî'?'r]ÇY¼?'ßî'?ïàœ0ˆð?dGžÎ¯t{?ocÏu°ª?dGžÎ¯t{AGN4FGL J1310.6+2449?î3)ß]¯@UG"…]¢sÀ:Œ—f¹rÀ<'Ã}˜²@ₓî‰á@o–Aö?»¯£½ú¿¥Ù«#ýÀ?ëᣦÙô@SqîYåO¿äêê>͛)¿Üº[_L¿ÛâCV–æ¿×¼Ù¥"cØ¿ì³+ ?:¨?Öôû?&£AGNbll3FGL J1310.6+2446CRATES J131038.52+244822.1?6?'Jö(ŸN?o*1N?'Jö(ŸN?ïÝ!™,â6?ˆBïô4­?qo3]à8ð?ˆBïô4­?î'lý¤c?œwÔD\È¥?­‰0/' Î?œwÔD\È¥?g(z•?xÓ;+?d?Žf("êÙ?xÓ;+?d?îÑ2tR?Ÿ	D§mÐe?¢ïÌÕPìç?Ÿ	D§mÐe?ï;Êm"?¨8µTjº?˜Ÿ†¹/Eš?¨8µTjº?îÊWÚ÷!?™'íï*qx?£^êƒ,tò?™'íï*qx?í;PÒÅ#?¢äà=©?³–%w²é?¢äà=©AGN4FGL J1310.7-5553¿ã_í¨†é¶@ˆ.¢ªºSÀ9§¢KïÃÀ;m$²>¬@B;䲝@SsD›:"?ÑqÉ—ïu?Ør­™+@Q˜ÿ?æ @o¦èa¨¼¿àïG€È|¿é'5deÛ&¿å)™—Ž¿ëüXáB¥—¿î¢‰,d?":#«š'AGNbcuPMN J1310-5552?ï÷ÜðRÛ<?M3#Jx³¯?PFmÍ·?M3#Jx³¯?ïâoüÆð?xÑøð<±?mµ@ú?xÑøð<±?îXÍm [?›¯[&<P?ªƒ-q}F?›¯[&<P?ïý?á
îÍ?&•é¬£^·?6÷_4œ?&•é¬£^·?ïöÇÏ?V9GhW(ò?RáØ)¦²Q?V9GhW(ò?îÍhå,ü?²/0m{Ƅ?£)q®è#?²/0m{Ƅ?ì•öpxý²?¥Üë¥kd?»PL|8t?¥Üë¥kd?ïñÀ㛬€?Q_'"Ž3?\~9IØP6?Q_'"Ž3AGN4FGL J1310.9+5514¿åGÞ&¢'M@NÔ
9À:[FóÚWÐÀ<´Näi¡"@˜GŠ®X@ÅP^½$¹?¸ÒK¼ÁçÁ?§gƒò¾N?êwAë\ÚÌ@ý;Qå¥â¿´XÿJ£gN¿åÓLãÞaJ¿åœ³"íbo¿åöØ9¦ë¿é¥ÖÏÛ¿ïýO¶÷xrAGNfsrq3FGL J1310.7+5515TXS 1308+554?ïü
'îe?7áPÐòˆ3??«æ"~#?7áPÐòˆ3?ïö²"²ò(?Qî®D÷V?RšØ֔Ðs?Qî®D÷V?ï`K?P3°‹õ›?aTs—uÖ³?P3°‹õ›?ïã2ùÁ;c?WÂv\°?lÍ)uJ?WÂv\°?ïòEÞª?RË´x\ýñ?[Ýt¾¼©?RË´x\ýñ?ïÜʙæ?q_Š©b¡¢?qš³Y}?q_Š©b¡¢?ï咔JWñ?sTkٗ1r?jmk—k ?sTkٗ1r?ï†Ló?yð	Q!+?ŽlüßbqQ?yð	Q!+AGN4FGL J1311.0+0034?í'WüdÁ@OƒqC9:´À:&­~Rì6À<Ìóc9‹@ Þ.Iš@þM œÃ?·ó;K…w¿¢!¹€Yé?éß[zz¢@7Œnbß¿âEU	FП¿×Oê£øBF¿ã{E†S¿àîÿA"¿ÜÓÄãŸL¿ÙT—¼Ÿ®AGNbll3FGL J1311.0+0036RX J1311.1+0035?ïù™Œé;?@`yÃD-S?I›ÆGxc?@`yÃD-S?ïîˆb©\I?e"3ºÏ?µ?awQ$Ví?e"3ºÏ?µ?ïì®wÞD?n|ƒ~+ï?câQysë?n|ƒ~+ï?ïònш¸?C"-Kq9?["]NÄñþ?C"-Kq9?ïé¼Dœðš?`>YÚ¢Z?fC»K²g?`>YÚ¢Z?ï½Óó2ù?‡'¢è?Š?€‹;2µ!É?‡'¢è?Š?ïßhà‹'è?x--ÝXÐ?pKž	À?x--ÝXÐ?﨤ïŽÛ?vãj1î?…ÖÄ-¨?vãj1îAGN4FGL J1311.0+3233¿ÔÂúªÅTÍ@TÆå6P&À9Ú J"cÀ;{Ø=CWn@®´2ø@.‡$L£?ÁÍÊùõ÷?ÐÖ\˜‡K@3Š™K–@IVå¿âÙ¿ë–ñÿ6V~¿¶ªåò7Àa¿ã,iöZe¿ã9ŠÀÏ6¿écÞAp ¿èØJCðð™AGNfsrqRX J131058.8+323335?ï±¥¥:±?´zŠ›áË?ƒ––¬Â§Ã?´zŠ›áË?ïów¦ª¤.?[oV"X?Y³.¨£e?[oV"X?ï-,ò¸õ?'p|¾X?šZa§83e?'p|¾X?ïìËÇX˜?Qjvºs8D?c48ã¯ð?Qjvºs8D?ï‡0qž?žÀ>Éª?œ|oZÆJ?žÀ>Éª?ïÔÝ܃gî?~AŠ'u?u'²]1?~AŠ'u?ꅮ‰QA?¬"ÎÛO.'?ÅéEÚ»Þú?¬"ÎÛO.'?¥¥t!?VÞ«ÀçR?Ž–¢÷Å?VÞ«ÀçRAGN4FGL J1311.8+3954?ã>c|@@S"Ú<÷À;‹ì §ªÔÀ<ñ令ß@ œÜl'¡?þɋϬ{?οUÀÑÁÔ?«fÝћ¿?àóîå%‰'?ýùö{œÙ?ïý'w>$ÿ?À7`"j[¿è™â"µ.K¿Õ4¸#G'Ë¿Ö<‹Á¿¨w¿äðÖÍÏ3AGNbllFIRST J131146.0+395317?ïþ8Iói?!¸
~o{?,{cÂK"Ž?!¸
~o{?ïðÑp9gÄ?]X‹U2àF?^]½—®?]X‹U2àF?ï鹝x©è?hælí|bW?fFbb:Oº?hælí|bW?ïØ\;PtH?ZV$³>_z?sÑâ?¬2?ZV$³>_z?ïþþƒ†»N?ý*À-W? Å_m¸?ý*À-W?ïÃ1
"R?ÁÆ±I?~gz©ªé?ÁÆ±I?ïÝݎ;¬?{—ï£yæ?q8Í×è?{—ï£yæ?ï?l!?‡p~w9ò?˜'}"­?‡p~w9òAGN4FGL J1311.8+2057¿Í?Ò9.†@T'(ÂzÀ:³ŒbÀ<k]Îpk@±ObhÕ×@
aûc?Åù‡€gny¿Àkí"ì±?ú
Â*²[1@"Àl—¿¼ Ì"Áé¿í66Œs¿ì£ÙŽ|/&?ºÕÊÍC?¿ïÿöùŠp?ì:G#ªÿóAGNbcuMG2 J131144+2052?ïôDÁ·+6?b2¬§÷«ø?Wv|Ÿh­?b2¬§÷«ø?ïn[ØÉ?¦hȪùõA?'<Ԟ\´Ò?¦hȪùõA?ïq±º'z«?ŒÓú,p:??'ÉȦñr©?ŒÓú,p:??ïóۍ¡?PýYzgt?XHå{Š/?PýYzgt?ïÜ«LÒõ?~†ùÅ* ?qªY£"ý%?~†ùÅ* ?ë ¤õº¤#?Ë÷êg'`j?Ã}l)ou?Ë÷êg'`j?ï7蜌H?"&†2¦ÉÂ?™ìu\ï?"&†2¦ÉÂ?î
!Û¶¹?¯yNý<w?®¯]å´0f?¯yNý<wAGN4FGL J1312.4-2156?¶‹=á7@DUóFí$À8µÁÉc‹ÁÀ;¥'õÉE@ýêAÞG?ý:61ë5?¨ŸCãÀÀ`?Ãc>Ò£¦@Ò­`ûH@¥ŠFjr¿áËOK¿ÍÐ-hî׿۠¾øN¿Ý^{ ۑ¿å«(m"˜¿êIÈ ÈdAGNbll3FGL J1312.5-2155PKS 1309-216?ïøTi?Rêk¬Àúœ?OŠ©"?Rêk¬Àúœ?ïÞâìé€?xÑ»h¤?pŽóž(ç®?xÑ»h¤?îÀ+FTÎ?šoÑÃ-q?£ýKFÔ#?šoÑÃ-q?ïòAh!žÙ?Ku-0_pƒ?[}0=óž"?Ku-0_pƒ?ïÓOöbrf?
ҝ@·?vXц}?
ҝ@·?ï+lÎƈK?³™0±?š'f*ž''?³™0±?îô:xæŠ}?™lKÂF.? ¼Xrs?1?™lKÂF.?ï¸Ó®úe?r+aôô†?ýAf¹?r+aôô†AGN4FGL J1312.6-1900¿ÙSQ¤7'@EÈÿ%¿­À:ê ú¶ëÀ<|K2-y¶@ …½ôAÛÃ?ÿ}"jŽ?©Â܉s?"†_ޕ·?ÅõÛĈ?ÿBX•~Í¿ë‡e_L—?ïóÜÁ6–•¿ÚÙ]ÔÇm¿áőڈw2¿ä†'ø»h?º)WgEžAGNbcuNVSS J131234-185902?ïýÓEóæR?$LVÿmïT?1eÐëWE?$LVÿmïT?ïî+°n-–?cӖ;Õfú?aÔOÆyk?cӖ;Õfú?ïî¥Ù)7Ã?e¥:>™´?aZ&³M<?e¥:>™´?ïëkL©É?P±ac֔Ñ?d"åîo~z?P±ac֔Ñ?ïúúòqnz?? ž&°‰é?D5먣h?? ž&°‰é?ï¨+¨Oiö?•Â\¯¤
?…õóº'?•Â\¯¤
?ïåºlMA?xºpò6ë?jE"µºnŸ?xºpò6ë?ï§/´Qè?vÑE«þo‹?†48Á½z?vÑE«þo‹AGN4FGL J1312.6+4828?ÝÙ@QÔªà"À8‹p*ÖmÀ;ÊPSÕj*@²6¡&Ö®@‡¤WÙÜ?¡HÔ|ì™?¯¾"¤9I@>vû	@ R3€5¿µùN`
VÆ¿ÜÆày§â¿ã%p'Iü¿áW^‹¦'¿æàTÔmªþ¿ß—ô}ë¾*AGNbcu3FGL J1312.7+4828GB 1310+487?ïýN÷MÜ?BdnÁ‹‰?5ˆCÇdÆ?BdnÁ‹‰?ï÷6«ދ?X'Y–`Q?Q'©·ˆ:Ì?X'Y–`Q?ïëBµ úü?iªZ•x|?d½J(D©?iªZ•x|?ïÿù1Q(3>ÁÁýáÝoƒ>Ë:-°UýD>ÁÁýáÝoƒ?ïýþ´/é?,Ϻj?0
^žÙ..?,Ϻj?ïß[ûSrï?rÿ¹1… J?pR?™Å?rÿ¹1… J?ïèׯÔÄh?s®2äö§?g(P` >?s®2äö§?ïÿû|R>¼NúÃüª>ÁùÒª2më>¼NúÃüªAGN4FGL J1312.8-2350?Χ(xo'€@Caÿ.Hè§À9»¤ûÍkXÀ<*b{ö@ 7™Ig¨?ûîPrß?¸ž·¥+?·í§¸Á''@eÂÒxy@Poĉy?í¾aÔU¿àR*ڟg¿Í'&]·Á¿ÞÅå"S·¿Ò‰ÎÒ`‹¿âÍ
>××AGNbll3FGL J1312.7-2349NVSS J131248-235046?ïúÀW•àt?:´ÔPO.?Dþ¢bOu¸?:´ÔPO.?ïèï9øä?få»ò4?gì›kôJ?få»ò4?ïæJƒ+ª?s'kuˆ—?iµoRu°?s'kuˆ—?ïÈêMë?`Îm+""?{ŠÙ"—b?`Îm+""?ïë$l,4?\т³Å?dñÛ«1#"?\т³Å?ïŸ<øÙÆ?—ÔÁ¤×d?ˆ:ð´'?—ÔÁ¤×d?ï¹qcÇ?†¢"ózQ?£¿ Þï$?†¢"ózQ?ï5[¶#û?…>C,†Ž?™T‰4À¨±?…>C,†ŽAGN4FGL J1312.8-0425?ÜúÉÐ0Î@MÜð0$À8åö1J%À;߬ÂkJ@ŽØ™´œ@¤u_þmY?¬wìÃÂ¥?Å'Øa*'P@[oŸË@hJã©K?臕ÀÇ
¿ÛAGÞeü^¿å¨ïbxñ¿ç¸Ž·«¿ç'£²ø¿ïÿK§ž?AGNfsrq3FGL J1312.8-0424PKS B1310-041?ïì,/w«¢?bŽci^£Ü?cÓЦíâ?bŽci^£Ü?ï팍—'¾?o8Û8¬a ?bsrDÁR'?o8Û8¬a ?ï«
ÚU˜Û?'o'Å$5ä?…<‰j™É7?'o'Å$5ä?ïþnõªz?Ԑªµð?)ƪž??Ԑªµð?ïîy˜kñ?]XX+D7L?a†hM~E?]XX+D7L?זּôÀ©?–'ƒ™Öj?"ÒBÂH8?–'ƒ™Öj?ï8ígª'Â?"¯àcõ¡A?˜âS†]Å?"¯àcõ¡A?ïû–°nè?4üã¦Îµ?A¥?"à'?4üã¦ÎµAGN4FGL J1314.7+2348¿ÚXò‰c°B@Tò	ª£­À9;Ñ|^öÀ;åw¹u4@dçv¯Š?þV½+o"?®t*a"ð?¸ÉÏAq9~@HŸ¬R@€\óvè?ïf* ºà'¿ßhøÑî¿Ý¡¼þ£‰‡¿à˜B"пâúK '\9¿íÍ;5À¬AGNbll3FGL J1314.8+2349TXS 1312+240?ïúÙÆ8Æ?SÕ¼F*#p?D˜çÚ§¦W?SÕ¼F*#p?ï±g-Ꮷ?ž7!‹]D=?ƒ¦4wÍâ7?ž7!‹]D=?ï‡ñÂê9´?‹ÜQÐ_§?ŽB÷	?‹ÜQÐ_§?ïpl'E.«?u"–O:?'òmÙø¨?u"–O:?ïö5öÔT£?U=Ô²ª?S"ÐHùŠ?U=Ô²ª?îñ—.7ÿ?®l'=npW? îv‹d²
?®l'=npW?ïwm{?'±Wt‡Æ›?'>ð˜¾Y?'±Wt‡Æ›?î|;1PÒ?—³Eà'…?®È<JW=ß?—³Eà'…AGN4FGL J1315.0-4236?îcÝbFF5@4O~ÃT~À:&¤/õ'À</ßÅoá@"`3F~j?ùÿJH"®?Á5Yh§m?¥$Y%¶?çoPð³[â@̪7Ìu¿ïù>Ú[V?îÉCu –
¿æMà}ٟ™¿ÖëDÜþÉ¿ÇÃdCK"8¿ÖA_›ÆðjAGNbll3FGL J1314.7-4237MS 13121-4221?ïÝøțÔ?®æaI?qÿ-Ò?®æaI?ïê@P°¥,?g/úŒØ#ñ?e¿¯H{›Œ?g/úŒØ#ñ?ïäÖì:Œ?tí(Pî?k)àãªëÄ?tí(Pî?ïò^PöÆ?GÚ¬€6t?[ïBâ`"f?GÚ¬€6t?ïîW
 9h?tEæ
m€?a¨õsg—?tEæ
m€?ï‹ß5žâ?"ªSZ'óß?2Š‰ç?"ªSZ'óß?ïÈ]nðù}?"KÆJš?{ÑHr=‡?"KÆJš?ïÇlCÜ4?pÈ\a•S?|IÞ#	Ö?pÈ\a•SAGN4FGL J1315.1-5333?ÈÆ&JA—¥@"HϧÆÀ8¦m¢šÊÀ;RáNd"@Ù{Üpê@‡½#â]?«AÔ&?À^GG@֜¾H'@÷¶p"è…¿Ñ慛
¿à†Àyt¿åUD€ª³¿æ(°B¨q#¿éh‹¬"q¿ê_Sb'½^AGNbll3FGL J1315.1-5329PMN J1315-5334?ïú2~,€¼?<í»Ê?G6Ú-F?<í»Ê?ïÛ ¦Nïã?}øqÛ­lã?ro¬Ì)v_?}øqÛ­lã?ïÒÈ8WN4?qK/ŸœZ?v›ãõU%¥?qK/ŸœZ?ïþ""Åø?^&"ƒBó?'¾7Òi͌?^&"ƒBó?ï傏«í?hþSØLY?j}pW!Ã(?hþSØLY?î™TTÀ÷'?´Ü#Öïœx?¦jº´Ìnç?´Ü#Öïœx?ïQTV¢Ï?'ç—Ï +r?•Õu//'?'ç—Ï +r?ïúEðè$?:ÕHßt"Õ?Fé¿Ê
Ð?:ÕHßt"ÕAGN4FGL J1315.4+8453¿ï772W|O@@?·¥ôÀ:ØÙ.IÀ<jÑâ¶C@xIéW@"}€^_1?Æ:azÄAc¿ŸÜŠľ?׳Ûåž@–ŠýtŠk¿×V^?&¿ëpBRŠçO¿â©å‡ó¿çÁ½ªE
¿ïÕ@%Nn¿í€MÍé,AGNbcu6C B132240+850531?ïú蛁ȏ??õÃ#P"õ?D]'¹¤ô??õÃ#P"õ?ïô|}í?Xñ)¯n¤?WãI¹Ö%?Xñ)¯n¤?ïº>Gckà?ZzJúõ?pn1ËÑè?ZzJúõ?ïê12/Ÿ?Np2v÷?eÎôА…?Np2v÷?ï÷§ÔšÌu?Q{0ßQ?P°V£ëw?Q{0ßQ?ïω¯ZÝ?uò€ä?x;(B9ñs?uò€ä?ﴕltƒœ?…¢*œ<µ^?'Ú¤êÆ3?…¢*œ<µ^?ïdößÅÍÕ?6Óàw?"a$m¯X?6ÓàwAGN4FGL J1315.5+1135¿ëKê¼C_@R]­BÃÉïÀ:" Rñ?À<eïÎY"Ç@ îRî'?øú™ú©v?É#–=áã?ËÐá.ƒ¡
@7°pu³á@Ôüj?ï)³ʅu¿í¹´V´A¼?Ì´ÆÆ£gú¿¿›Gn©€í¿×{°&äp¿äÎK^˜AGNbll3FGL J1315.4+11301RXS J131531.9+113327?ïû¹I7W?6­4Üà5²?C;´ÆÐ?6­4Üà5²?ïærÓå£f?v¯"ýXÊ?i+ò"9?v¯"ýXÊ?ïå×m9¿>?d€‰?hÒ{?j('Æ@Á'?d€‰?hÒ{?ïç)hj]Ó?PŽÅ,Pà'?h֗‰C•?PŽÅ,Pà'?ïö"tng?P;u2šN¦?Rz÷'WŸ?P;u2šN¦?f®?–ò6ÃÕe?‡æq˜Üv?–ò6ÃÕe?ïÐY¸ò¿?y¨Ù*ÂÛ?wÓ#iÒ^?y¨Ù*ÂÛ?/åˆ&ø?qfÁó…iP?€Ü'?´?qfÁó…iPAGN4FGL J1315.9-0732?é"Ûƒ7Ç0@Ki"}ŠÀ:
뱔b"À<(^Ì>1"@ƒkµ/Í"?üO9#7=?¹…cÂD¯?Á·uø®@.d²1@@mdDM6ê¿Ü$´?b@'¿Ù²ÕÎÂE¿¨ˆÕü÷7¿ã!¡ŸØx¿Ýa'nê¿ãwקò"AGNbll3FGL J1315.7-0732NVSS J131552-073301?ïþŒÍÙ<G?Ètt´?'3%¿A4F?Ètt´?ïò|[	)ä?aeë®ò–À?[I|ùk?aeë®ò–À?ïê¯-L
è?d.oœHŠ-?ePÒÖQ/ó?d.oœHŠ-?ïýs X?`Ô¯¼P?4býªßÊ°?`Ô¯¼P?ïûx!Wq4?=±­Ó§›?B{šN?=±­Ó§›?aG_²e?…r]úãà?€Ÿ®(k\Ü?…r]úãà?ïËòþSœ?}ædÍóŸ?zp'TQÂ?}ædÍóŸ?ïùN^÷v?9Î4ӑÔ?JƄ-&¡Ñ?9Î4ӑÔAGN4FGL J1315.9-6349c¿ãì:¾l⬿ña၏·™À9ªl…dXoÀ:²/€ KÐ@'±…"@šTÅT2‡?Ò§9)í9T?ºM6iž2?äkž´‹g@T,Ž~]~¿ïüœž0Ø?îï7œ¿âöÙÑ.[¿â©‡¸Æ…‹¿éUDÀyWZ¿ïðdìé¢ÆAGNbcuPMN J1315-6354?ċŠ¸?š'š˜åª?ˆßÎàŒíñ?š'š˜åª?ïÇGJt÷?‹û=2{ã?||ÜJ÷P«?‹û=2{ã?êìG@RÍÐ?°LºÑt<Ã?ÄNâþ´ÈÁ?°LºÑt<Ã?ïÁx)ÿ¥4?jë‰@¨?CêàþZ?jë‰@¨?íÃK
j÷?¶ÃðSfcÊ?±å§˜˜D?¶ÃðSfcÊ?îig¬PoH?·Ë)Ê·p?©i…9A=ƒ?·Ë)Ê·p?蛄ø·!?³–¯ö8')?͑ì½#{?³–¯ö8')?í_½ÐZ à?¨±ú/"Û·?µ~ßü?¨±ú/"Û·0AGN4FGL J1316.1-3338?ãY}M–®@<ôFs×ÜÀ8gõò`MÀ;ˆÏ×CHT@Ÿ­"Þ@GØåó?¡õ'	^Ú?²˜Pï0Ï×@c3á®Ü!@…Våb¿ÐÒ¸©)¿ÝÖ¾=<÷W¿å3¥´Z@¿å¼ä!}(J¿åUK Â€¿åZ‡5DAGNfsrq3FGL J1316.0-3338PKS 1313-333?ïýòºzÃH?"ï9Œ'?0j*¶C2ý?"ï9Œ'?ïón'û®ž?["²i´?Y"ùš¯E?["²i´?ïæ"2C
?mš+,Ü?i{͕~u?mš+,Ü?ïÿ³ǘ>öñ•›‹Ä?>.FIó>öñ•›‹Ä?ïýÌá‡Ó?+d£¨µˆ?1˜ø
ë?+d£¨µˆ?ïÃ8ÂûMû?pΦ?~cžŸ5ºu?pΦ?ïÅpšz?ÿ8h©ó?~={­•ºë?ÿ8h©ó?ïÿl³Ì9™?
ܯnYT?i‹\mË?
ܯnYTAGN4FGL J1316.5+3013?㩏PÈøà@TëQÕQ×À;¬ˆô'À<ÿé]&KÄ@e°ŸÅ'¬?ûÒÂÊëK=?âÀžìå?қ‹vÁ'}?ö;¥wô-d?þ•ùqE'†¿ïý.)7?ïÄҗç貿ìV́¨Œ&?Ӑ¨"C3¿çZüۈQs¿ïÿ^Ô÷"AGNbcuRX J1316.9+3014?ïõ¸æ9Z?Pš wû¬b?TùéU»"?Pš wû¬b?ï³¼€EØ?—Tؙ?ƒ8Óçè?—Tؙ?ʵ¹?'€Uh¥Ðq?‰ÍEa¶?'€Uh¥Ðq?ï®Åõ1Ð?q¸£bø?"N'ªãú?q¸£bø?ïÂÂ4Ò?ˆ­('ø}¼?~žþ"ì¬?ˆ­('ø}¼?ï>éRrY?¬SÝÆÆÙ?˜"Õ³tbÞ?¬SÝÆÆÙ?ï$º"'B?'ÜíE,Ú?›h¾4¢Ç?'ÜíE,Ú?îy¬ºJ®? oƒ}lu?¨e>…7< ? oƒ}luAGN4FGL J1317.1+6613?ë'ëòyQ@IYÝDUGÀ;D·éæ¹À<ÑÜKÅÑ0@ƒÁRñ©@|l—ØÏ:?ÂFµœ¬2¿§¨¥ûý'ç?âN¢?Zˆã@ÚýA‰¸%?î†@áDž»¿âk
ÀMb‰¿ê

Dý`¿êjˆ¿¬¨À¿ÝAÞò"2?r<TçZdAGNbcuTXS 1316+665?ïýgÛl³ï?/¨|í5‡²?4Á#'lØ?/¨|í5‡²?ïõûjw ©?T+G¨Gs½?T	*­Éîs?T+G¨Gs½?ïÜ:¾öS?p5¶Í\kÈ?qâ n)P?p5¶Í\kÈ?ïöÌëU£ö?:U­ËC¤‰?Rf)¡¯RÂ?:U­ËC¤‰?ï÷Bäx‡s?PÌ 6L´a?Qz75lº'?PÌ 6L´a?ïÓ_ƒHIp?uö ?vP>K]('?uö ?ïÄë‹#p?~/#!ÎÌù?}Š:sžÔ0?~/#!ÎÌù?濾Ù:Â?xûÑ`ôü0?†^É»ª£s?xûÑ`ôü0AGN4FGL J1317.6+3428?å`ó¹~Å@T0Åë1;âÀ9ʵ™ª`'À<jz4y"P@yáäáìo@÷
=p£×?´Qbޜƒ?´Ñ^¬ÞšÖ?üëNbc¢g@Vð|ªK¿Æ!Ï4`¿å};?HÜ¿æÔXÖZë¿å¡ŽàØóL¿í+™
þ`Ä¿ïâfê%xAGNfsrq3FGL J1317.8+3429S4 1315+34?ïûHÏ?^aHâÍ`5?BÝý
þF,?^aHâÍ`5?ï÷®é´¡?TõÖG~%–?P¢-§Ü#?TõÖG~%–?ïâ¸Ó?s«ißow>?mGîüÙw.?s«ißow>?ïú†tßâ?6 ØÔÖ?Eæ-|AŠÎ?6 ØÔÖ?ïü¶Jƒ,?1¿Ëïßê,?:M¬ž,'?1¿Ëïßê,?ïބð•(ò?uʯ Ìv¹?p½‡¦ý+L?uʯ Ìv¹?ïã(µÅŽ?v1QãuÑV?l×J7²M?v1QãuÑV?ïñhfàx•?O€ÑZ¡–?]/2ÂÿÕG?O€ÑZ¡–AGN4FGL J1317.6+7450?Ԍ°ú«¤«@E<³åuÀ;'mÄÿxòÀ=ŽVox^@W"f1bN@_^4h½?ÏÇíÕ[È?Æ(t"OÓ}?íëù¸¾"?÷õ±Ím¿±â˼¬n3?à:õ¿ÏÖ"î9.¿ä©L•£¿çë@àðÆ&¿Ó~/?‰AGNbcu6C B131714.7+750402?ïöZü¿~?Qôºá€J?SJ ôS?Qôºá€J?ïÇ"w³?ˆÒ¯‡9;?|@ný³"m?ˆÒ¯‡9;?ï‰ýEÄ?‹·òO\Aq?¹ú¹ÏW?‹·òO\Aq?ï)Tæ>ìX?zé7Qå?šÕc=Iß?zé7Qå?ïæ7¹Í
1?i¼ÏC?iÈF6ßO?i¼ÏC?îÁÇÇÄ/?­J1hש?£ãƒ‡.i?­J1hש?ï Ýë$ž?"hgŒzÏ?›äBžÛÙÍ?"hgŒzÏ?ìceêâÙÌ? ²®÷ sÃ?¼äШé1¡? ²®÷ sÃAGN4FGL J1318.1-1740¿ä=dSÞñµ@F]6Þ¹^[À:º¸ÌdÈÀ<fèQ'N@ìË]ë@þÑa‡•?È~ÓD¶?·—
ž¦Ñ?í;Ì^èã@¡ Lü‡û¿ê=G‰+M?ïëÒá长êÀ|1¿Þ¼ŒxHæú¿å)+<Ĭm¿ïÿóÖ&ãAGNbcuAT20G J131808-173536?ïüâÞJèJ?0?VQMT?8é
pªs0?0?VQMT?ïì,÷.ö
?nìt¼!OL?cÓéÇ#'?nìt¼!OL?ïé<ÊûU?]"•"úh?fàÃ[€J?]"•"úh?ïíŒcâ9?HÅ0"t%<?bãsÌ8Nç?HÅ0"t%<?ïð÷Þb:L?dU£·1?^BÞ	M?dU£·1?ïäôO·g?™Í»å<èæ?ˆ†ÂùЖ$?™Í»å<èæ?ïÊ÷Õ0•ì?€ÔµrìÈG?z"x3)º?€ÔµrìÈG?ï"@R;È>?~ ç‹"ì?Šïë_ßä'?~ ç‹"ìAGN4FGL J1318.2+6754?î½úü#ì2@H±Ù+áÀ:âñ#ôÒÀ<ö1ø .@ʁðÛtÛ@"d¼B;?Ä+þNå?Ê'€EŠ¤@aãðÕÁ@Ÿ
qÈð¿Þ˜L<™Ž\¿ÑëŠ<¯]Ñ¿äiü¾, ¿Ùº?–më¿ìE ž²´¿ðAGNbcu87GB 131701.6+681031?ïóðhÄuÌ?T"<å<pü?X.øE¶j?T"<å<pü?ï÷Uà9ï™?QÒc`‰Äñ?QT?Ÿ^ž×?QÒc`‰Äñ?ïÊhwi?‡:'»};Œ?eì‰y¾?‡:'»};Œ?ïül°{?$ÿKO3ÄÔ?<œŒí…Ê?$ÿKO3ÄÔ?ïö:`ñSâ?Pào"XÒó?S‹=àß?Pào"XÒó?ïá0íÕ·?pmžÿ3 D?nÏí+ˆ¸?pmžÿ3 D?ï
FIï?•î©1
e¿?ž>¼î ?•î©1
e¿?ï÷‰¹ãÍ?C6G€©æ"?QÄìñìÕ?C6G€©æ"AGN4FGL J1318.7-1234?䆈jûª@HÞÆÞvB|À9ÏhµËÿGÀ<BÛ·K[H@Õ'*g@'Ú˜gjr?µ¡N›Ä?²²Z@úW[?ühMÇ3/Ø@©vƒ¿èŽ?ïûv=žñó¿ß%ôñ¯e¿ãÚüȼ¿á{lB†Ï¿áÈJÕ¿ìQ›žV—¼AGNbcu3FGL J1318.7-1232PMN J1318-1235?ïý¡(/Z?$Ë@jRv>?2÷ôª[JF?$Ë@jRv>?ïð@äe‰‹?a*"ÄLQ?_~7aˆ?a*"ÄLQ?ïôG"Ώ¬?X8!Ê¢?WpصWH
?X8!Ê¢?ïè‡ÄÁ Ø?Nùø'Yõ?gx;0?Nùø'Yõ?ïúwqMÿ?>{g9vA¿?F#•px N?>{g9vA¿?ï»+"©´U?•o1G=Ö?57LûäÆ?•o1G=Ö?ïìôI=Œ?rŽƒ‹‡ª?cî‰gœ˜?rŽƒ‹‡ª?ï°wP2a@?o7¢ñ?ƒâ+ðÿö?o7¢ñAGN4FGL J1319.5-0045¿í҈äs:=@N¦ùü°À'À:nd-§8À<lf/	@ؼKV@G@ÿ¤?»L·Ñ=ö¿‰ò'­gë?ÍåÑ*ªx@i?%3?ïü¹>z¿äAèÜy¿æŒížÔký¿áXl"h	Õ¿ïü#!BDô¿ë‡ù(ujAGNbcuPKS B1317-005?ïû»h—Ä?;lÄ*½	?A®ÞE'{?;lÄ*½	?ïó²P@?Zr·$Ê?X›`BÞÀv?Zr·$Ê?ïÕ]]0æ/?y"	½•ÿ?uQQ‡Ù<?y"	½•ÿ?ïú.3¼gq?4Ü'¥{2•?GG0*<,?4Ü'¥{2•?ïø¾ ü=Â?F6N…<`?M{:ÔJ'?F6N…<`?ïÉ)\Î?Ç?ƒhÆMŽÌŠ?{kQ—€Ds?ƒhÆMŽÌŠ?ïßï‡ju?yh±ÝAÀé?p<dâ9:?yh±ÝAÀé?ïñPx"N?OŸ@70€?]_qÅd®?OŸ@70€AGN4FGL J1319.5+1404¿Ù=?Ë
ïŒ@RؒyèÀ:Ó!ž¶9À<™>ÔI™@øËagÏ?û߶må·?Ïâ+™5ñ?ÐA´ †å@¹	k¹Œ~@v®óH?é¬
¥0ç¿èæä:§›»¿­÷Àkj‡2¿á(ŠÎ$»¡¿Õ/æ5T¿ðAGNbll3FGL J1319.3+1402RX J1319.4+1405?ïûqŸ÷Îû?7""T±?B9"F,?7""T±?ïã­¬v0?xÆíüNšð?lRSJ²E?xÆíüNšð?ïÔTJQF?t¬ø:¬D?uÕÚ¿3#?t¬ø:¬D?ïç̏\¡8?N¿à³º?h3p¯½_Ù?N¿à³º?ïû><+]??2Ç>&Ü?C¿ä ±0??2Ç>&Ü?ï—vÈå? `¨í•e?Š"y"¥ð¾? `¨í•e?ï³Jé	?ƒÜBfÑù?ƒ-E°Pѽ?ƒÜBfÑù?ﭑ{=
'?t3n2ãN?"›¡&mâc?t3n2ãNAGN4FGL J1319.8+7759¿´Áç(÷"¿@C"{¢7ÍÍÀ:)6&,ºÀ<ªÖR5W@¾Ë$V ž@Y©qÛ?²"`_;Ná?Spaù.@
‹éû†Éˆ¿åÐ!ÙC©¿Îd"i®ðC¿ä΋魮$¿àU<þ
6Ÿ¿ßÐ`zn±¿Ö Uu}ZŸAGNbll3FGL J1319.6+7759NVSS J131921+775823?ïþÇC©€ ?¿ü±6í?#‹È,â~?¿ü±6í?ïøkݯÚ4?ONoþ¿ñ?NPŠ1 ?ONoþ¿ñ?ïù2[që«?Fü#18?K6'EƒS?Fü#18?ïý"3ř?!bÚi0|?3Þ`wŽ!?!bÚi0|?ïþ{R~‹?Ԙ»-ˆñ?(JÕF6ے?Ԙ»-ˆñ?ïޒ4?q`†HöX?p¶öd§?q`†HöX?ïø¬0—né?c‰FnÞì?MO<¥aÎ?c‰FnÞì?ïúÔ^³áç?6.ä·'³ž?D®"'—Bâ?6.ä·'³žAGN4FGL J1320.7+3314¿ï™Ìð3.V@TM*®)s—À:ÖÛÃ	ÕlÀ<€ëLê"@êØ¿IV‹@g†
¢?Íía—ÊŒ?Ò±×~¶ß?ÿi±Y©¿'@(¡ ¤$ã?ì†X>…vÍ¿åÎj[¾l¸¿å­u"›Y¿ëÞ`]Ï·¿àù«ƒ¿ïÿÒþÀùAGNfsrq87GB 131814.4+332742?ïûát·?H\d['?@{âá] ~?H\d['?ïõxb<`.?XF«õŒ•—?U;!‹5i?XF«õŒ•—?ﯙåç|?Zš_¥©?"†wr)?Zš_¥©?ïîµo¸õ?Hëâ‹Âø?aJuÅ0L?Hëâ‹Âø?ïü˜ã¢b|?<iÿUxMš?;8ãND¡?<iÿUxMš?ïӐ†~†?€¤.·
Hï?v7¼Ò%H±?€¤.·
Hï?ï,ƒ¤?•þ"œï(?šoŒS*·s?•þ"œï(?ï Ü­x?w̛^s³k?‡Èùƒ3?w̛^s³kAGN4FGL J1321.1+2216?çÈÞµ54@Tlºˆ&«À8ŽÅâÍÀÀ;°…ù©¤ª@ï°¨ÔÊó@@gc¼gû?¤)0N&v?³Ú6lΊg@Î^'lVj@rø_¢¨¿ÕÚj$"¿àđ"èYñ¿åG˜_ݶ)¿åž@ÈG,¿èÞê¦ÒgA¿ìJˆ_	¥ÆAGNfsrq3FGL J1321.0+2215TXS 1318+225?ïýøNð«?1.*RK?0=a»^Ä?1.*RK?ïóÝ:XA?[çI,É&š?XüEb/(?[çI,É&š?ïÍØ
?w—Ð}CÀ$?yñdáÊî?w—Ð}CÀ$?ïþ—¦Y?€/Íd'¥?&…¤B?€/Íd'¥?ïýjîz5j?2›#ð6-?4¨‹1qq?2›#ð6-?ï»"±f?!U…Ü?:¸š´r?!U…Ü?ï»Ýè9K?"_ddªÂ?…í5¿'?"_ddªÂ?ïüEJYaè?42Bq°¨?=Õ®Šãt?42Bq°¨AGN4FGL J1321.3-2641¿ï±.€Æå@AØàÉÙÓFÀ:ب)À<L[œÞÈx@bó•8Œ@;þ¦c¬x?ÀªãƒrÁ¿¶B³-êI
?öª¼¤¡5@Tä©~>¿Ï""ÜÉ9¿é1àþ¿ì'ð}V¿ŸPg˜âÜÑ¿ç ÕÍýNu¿ï÷ŞÛ!úAGNfsrqPKS 1318-263?ïÏa›Lø?¯B"°Àl?xOt°IÀ?¯B"°Àl?ïå–%'Ý?q:Y"ãúp?jiڏÝ?q:Y"ãúp?ïÖߘ+…j?l²F¦²?t4yÚå?l²F¦²?ïôښÀ¶?B"õ!Cò?VJÊ`WIæ?B"õ!Cò?ïÜ+©É^ü?ru/µÚ×Ï?qê+'NS?ru/µÚ×Ï?ï"ÁæóG>?'Wm%ý}Š?ŽÏ†J
h"?'Wm%ý}Š?ï™nýàb?‡\Üч?‰¤z¹¨¯k?‡\Üч?ïb¥4f?‰òŽµé?"«_×»o+?‰òŽµéAGN4FGL J1321.9+3219¿è–"tˆà[@Teˆ±Ù+À;IÀÜԁÍÀ<¸Hi%]ˆ@»Fc'ŸÐ@À
¼%/?Ål¡«¶Ó¿–[߂d§R?ÔÌÎzKö@ä*m'ÓÒ¿åV…þ\;ë¿äæœau÷¿çSˆ]‡º¿ÝVÀ	¿æ\C'‹¶?‹›Q:ìKAGNbllNVSS J132159+321903?ïþÖÔQjE?`ނ†9d?"'ºëŽ¨?`ނ†9d?ï÷ãc3£h?S½s¤K©?P99Éí1s?S½s¤K©?ïùÄSEf*?>Àž¸Ð'?Hî²%—Pê?>Àž¸Ð'?ïú¼dãp?0"_Ÿ…?EoW]Ƴ?0"_Ÿ…?ïýΦ°r=?(ÆÐüôLÊ?1ŠÉÄÏÆ?(ÆÐüôLÊ?ïÚWÈÏù8?ž#7yF?rÔ}6oÿ?ž#7yF?ïøGµ~Û?Z>c˜R?Ná)ùoQ?Z>c˜R?ïߙ¦ç?cEp7¼?p3y¨:?cEp7¼AGN4FGL J1322.0+8317¿é<aÖÅÛ'@@ã×<'W†À:\Û¦"c§À<@–ÉÁ@!š…Ò½R@èJה§?Á<´ÿ?Á¾z¤‹åý?üà·õ¥3@Á?à뒶?ã;xçrj¿Û®qÊG·¿æžÍë°½£¿àÁJ³οëù®AÇJ­¿ïýR†Q¾AGNfsrq3FGL J1321.7+8312S5 1322+83?ïü‹ vqe?09
b‡'?;¢ý›Î´x?09
b‡'?ïöã= ?VÍ#O˜¶?SÎ9L'€Ò?VÍ#O˜¶?ïÝ16-äj?pÈUÂE߄?qgeÊú÷?pÈUÂE߄?ïûy€ýôì?*R¤W*»Ã?Bü'8V?*R¤W*»Ã?ïøL€ÈM?EàÊÏ8÷Ò?NÍü!›Ú?EàÊÏ8÷Ò?ïÙ7
Њê?uBIœCQ•?sdz"Jï?uBIœCQ•?ï¶x'bî?",¥w¸¼&?'aÛoƒlÆ?",¥w¸¼&?ïõ9!¬›?D™Ä¬ò4?U¼UV)Ë?D™Ä¬ò4AGN4FGL J1322.2+0842?åðނŠfÿ@QŒ2 f<uÀ:gég7F¾À<~ˆA'O@k‡}'@_`'÷–¥?¾&4ÈÂÇ¿—©Ä—ÌÝ?Ú5˜}ºÀÜ@"{½™Á¿Ú¯Þ|·â¿ç–œŸ2ŠÂ¿â.5!õÉ¿Û:…M\T¿ìrH½3«¿Õ±$ûŒÿAGNfsrq3FGL J1322.3+0839NVSS J132210+084231?ïúa2Iÿ(??ºo˜Â—?F{6,}I	??ºo˜Â—?ïõO¡Â¡¿?WzÑyÒ k?U`¼Q1V?WzÑyÒ k?ï¼N¨¿¨?€˜ñðÊ
V?€ìVÆ£æ?€˜ñðÊ
V?ïýás39¤?!2K­J1?0ôfŠ‰"?!2K­J1?ïôF^'¹Y?O[Ê@q?WsC1Ý?O[Ê@q?ï̆7Uñh?7w4ËU?y¼äsóÇ×?7w4ËU?ïÍ»»
5A?·}®Ï/V?y""vë®?·}®Ï/V?ïù·.*	ê?<ÃkpڒA?I#G»YÕ`?<ÃkpڒAAGN4FGL J1322.3-0606¿ë_×"ˆ@K÷²VÿÁÀ:óY'BCÀ<´¡õˆ­¹@@ ?û4ï*Ŧh?ɂ§Í"]?Ö¨B¿BJ¨@3å	Út?ÿl¿y'3¿ïÿúVrÓ\?ïÿêњ'ç¿Ô	B%¿ÝjwØ~±·¿âYDàá6¿ïý'Æf>AGNbcuAT20G J132219-060619?ï;–šÅû?•~ß¹l%?˜?̧@ª?•~ß¹l%?ì'we'+?½Ìþ¶Sä"?¾ÄDÓn§~?½Ìþ¶Sä"?î@Õugá?ÎC÷$?«ò¨§Ê!?ÎC÷$?"+.?ˆ'ù¼—?¥׸
M?ˆ'ù¼—?îCÏ/I?©[1—ç7¾?«Ã_£°r?©[1—ç7¾?âHå7Ò?ÐârK!œ?Ûn5ّè\?ÐârK!œ?è	^äo‰X?¶ŒŠ?(?ÏڄnAڞ?¶ŒŠ?(?èF6OiÂ?²?Øp	¡?Îç&ÂX÷à?²?Øp	¡AGN4FGL J1322.6-0936?¸gûíÅÂw@J?^g"dÀ9.ø6#
À<"*M±c»@SoЍ@'êÓ²š?­Š¿q6	?¹¸A¿+é,@û#š8ûÊ@«AOÝ8¿´"ôxA¿ã¦¡Ÿ¢r0¿é,.âkšƒ¿éŸÎ!5¯º¿ç4R¿æ@Î&i UAGNfsrq3FGL J1322.8-0938PKS B1319-093?ïþ덭'@?GÃÙ*Ë?!G&¿÷Ö½?GÃÙ*Ë?ïóQEdZ•?a
Nxäf?Y]u)Œf6?a
Nxäf?ïå¸ÌÃEB?oZ´öO#À?jG3`v­œ?oZ´öO#À?ïÿª´bâg>ùõ#Œ¬?Rà?·öë>ùõ#Œ¬?ïþþ$€	r?!nöÂAEß? ¹ª)l?!nöÂAEß?ïÂÐ7÷yZ?"y¶;o#›?~—äð¾é?"y¶;o#›?ïÁ9˜`?€Ìï"ÈX…?cR,ßè?€Ìï"ÈX…?ïÿ;XŠt|?kGÇC?"ð£¼çï?kGÇCAGN4FGL J1322.6-1418?ïÝTovŽ@Gð*#¿ø©À;wëÒK'ÏÀ<°$?ziS@ d°êöY?ÿ)¸`.>?ÑÔȄ=¼Ï?Å´!ZBÁœ?õGuàVíM?ôí¡
Ò
¿ït†ŸÁÑÇ?ïüÖ 
L	¿âL€ Ì©;¿Ý3<mn˜¿äô'Þ½¿âÍÐØËÑAGNbcuTXS 1319-140?ïû*½1¾??Ò5¬8ý/?CUJ°??Ò5¬8ý/?ïTjfñÕ?˜ÐôØ7A¾?•r³F€ýG?˜ÐôØ7A¾?ïÕɵ
?sÀ`óJ:?u%Šÿþø?sÀ`óJ:?ïlœØ,@??wž{<¡šê?'leþ ?wž{<¡šê?ïù5=
ë?F.ÁG?K+@ÐøÊ?F.ÁG?ì
4ÍÖÑÍ?Ãú±à?ùÉ?¿–Y'Iq—?Ãú±à?ùÉ?ïºæãE×r?ƒ7%0"'.?FG%C1‰?ƒ7%0"'.?ë{³³²ZÂ?«R\0gë?Â116"ù?«R\0gëAGN4FGL J1322.6-1617?íL%$9É@FöFñVÀ:½i&4G/À<€SM"î@FÒ̖5?ÿ~"ÐÜý?ËÈÕFmø?»@ö•H&4?ñ%HĔïç@QÉc?ïñÑ~N³¿é§ùä]K¿à/÷¤ç«¿Ödf[ÿ…1¿ãðý=ØӖ¿ïÿøãúAGNbcu3FGL J1322.6-1619PMN J1322-1617?ïüO(S¨–?2Ïï fQŽ?=†½yÒI`?2Ïï fQŽ?ïîk­?]o.Ê5sJ?aéåW[?]o.Ê5sJ?ïïvt?[Ï?WçöDzŽS?`‰‹)Ð÷?WçöDzŽS?ïâ7%ÂB–?MëýH"Ù"?mÈÙý$Áö?MëýH"Ù"?ïýEZÓ
T?0FTù°žW?5Õ*üL-ë?0FTù°žW?ï²2žà?–s‡Ò•æ;?ƒsXr ñÿ?–s‡Ò•æ;?ïïzŒÁ¢€?i8o"Ù²Œ?`…s}–OØ?i8o"Ù²Œ?ï'(WG˜?s×ã2•*«?‹µù™?s×ã2•*«AGN4FGL J1322.9+0437¿æQ7†ÈO@P'ò{xÀ:ïùwO¶À<™€TN5î@ L—ú³?ùnˆwÆ?ÔCÔýKp?ה&}˜1:@2äÄ:W@ʨ<ʋª?îÜEæ"0¿ìõ΃†1Þ?Ïb`\â@¿ÂôƒJ!â(¿æ5'ST:ë¿ïñH­ûŸAGNbll3FGL J1322.9+0435RBS 1257?ïüET6Ó?A´&ʧ¡B??
Õàv#?A´&ʧ¡B?ïãPàÿE?tŒ Õª™U?l¯Ö×ð?tŒ Õª™U?ïÕ|tMbg?oÞenÎM®?uAÅâí´p?oÞenÎM®?ïÆ*̇W£?cèeTyœ'?|ꙡ‡:Ñ?cèeTyœ'?ïü$º–â?<B
XˆÆ??öØ]}uS?<B
XˆÆ?ï¯U¶úc?ñkL0-?"*'"Y1?ñkL0-?ïÒC%2ƒO?}&K%½´?vÞmT0t¸?}&K%½´?ï5E9΋?€1)ù?WUV'—?€1)ùAGN4FGL J1323.0+2941?'à~aX*@T¦}¿H€À8è[;ùÀ<ʍWkø@9Dü3l¿@êKáQ?¤p½¾x1{?«²DœxWf@œÄÇDÎ@º`@²w·?Ç2"åX¿ßð(‡ƞ¿ã½†]ҙ¿áŒé½ž[ ¿å>¨²;Q¿åwR|¤–MAGNbcu3FGL J1323.0+29424C +29.48?ïéÿÇJƒ?aZ¨82p?f9'4Á?aZ¨82p?î×(R•¤?¯̬*:È?¢ØBðÂ?¯̬*:È?ï+áVœš?•R&f¼º•?šŸÃÓtžÈ?•R&f¼º•?ëRþ#J̜?­"–'»?´rÔ͑?­"–'»?ï.u$U†?œc*ï-O
?š1[qߤ?œc*ï-O
?ëmòÌ»°?Ç1¿¸oÑ?ÃÞH4Í@?Ç1¿¸oÑ?íö' %FX?£ï+*&úS?°KêýÿC?£ï+*&úS?àoîDÁ¥ý?ÀÄÎ9!C?ß #v|´?ÀÄÎ9!CAGN4FGL J1323.9+1405¿¼wó&þœ@Rº×à&EåÀ9æO"}ŠÀ<3PëªÞe@ cøÍܗ?û9AŸÝ€y?¾ÏiŠ2H}?Á­wÝ\<@í†"ÄP'@¦©øa{?螺¯ÀLŒ¿ä—P~"Ñ¿Þˆ…3[!¿Ïñ[øNZ׿ޠÁÁ€éJ¿æ/RY,AAGNbll3FGL J1323.9+1405RX J1323.9+1406?î¡%éëãá?ÉÌ=هù½?¥í¡`eÚö?ÉÌ=هù½?ïë?—Ö²?qN¸&!ÿ¼?dÀh?KpÊ?qN¸&!ÿ¼?ïÎõÜ?…ëþ'Øå?xóžùòU?…ëþ'Øå?ïð³(X[-?Cj^ï'få?^™¯¡ÀE?Cj^ï'få?ïû*'hF2?;õä¿Z?CWc@ÚT?;õä¿Z?龜ƹ7?•e»¤9
p?†ÝþÜ"?•e»¤9
p?ï wO—Ã?bØùgÒ?‡ùb!Ë;Y?bØùgÒ?ïÔ¥™à™ç?cíEJ?u­2öEð¼?cíEJAGN4FGL J1324.0-4330e?Ñ¥\QJ܃@2ú&€IRÀ7®Í™{f©À:ØÆ;¹²@D*Se­¯@Äw¡!MX?£®¡†­?´-2<@à
quŽ@ô‰PKFû¿Ú=1cÐ4
¿ä+ïý©c'¿ç9m	Ö¶¿çÓÞ¿=˜¿è˜—;ˆ¿ç04{1ÐAGNRDG3FGL J1324.0-4330eCen A Lobes?ïx$——"d?²qÒ?ûm.;~?²qÒ?îÍ|h9?«…ïñÿ‡?£(9|o߃?«…ïñÿ‡?ì[¡Á±:Ë?¦ŸÉhÒ?½"ñòv)¨?¦ŸÉhÒ?î2y5º»Â?™¡¥ãœš?¬Øl¤TCà?™¡¥ãœš?í¡Š&†§?³+6¼?²ó¯
ðF?³+6¼?ç¦Î€¬ä?ÏÝ\KÁ†?вbþ§æ9?ÏÝ\KÁ†?é`y× R?²£Ô¡
ž}?Ê~£~º?²£Ô¡
ž}?ãÏ6\f?Âeó9sH?Øa"G3ßð?Âeó9sHAGN4FGL J1324.9+4748?ç)ê™çG@Q³AáKàÀ:A(Ñ°aÀ<lÖ#£Â@+»öÀ'@#ˆ?¾äaéÔð]?¬PÑÿ'›?é"x¸xò@aŸ~àÛ¢¿Þ}³¿µ¿èüØÎbÏ¿çtøÀEªÚ¿ç8uý³¦¿î'âJãS!¿ïýNª‡þgAGNfsrqTXS 1322+479?ïýš¨y
?$ö#j¸º'?3*¿~‡ÛŽ?$ö#j¸º'?ïøz<SÁ?V'r-ñŠ.?Ná•#?V'r-ñŠ.?ïì"\?X¿3Ôö
?cøå—d";?X¿3Ôö
?ïýêbE*¾? ¸Y»dë?0¬í¼F¬n? ¸Y»dë?ïþ{k¹À?"Êý"­§?(IAªèX£?"Êý"­§?ïߘ	²Âq?rúá:º?p3û¯Ë°?rúá:º?ïð;ʺ ?fddߢ?_ˆj#Š º?fddߢ?ïù¥[L_ˆ?><AZƒ{?Ij"!…=£?><AZƒ{AGN4FGL J1325.5-4300¿´ï­S^¤@3k8''À7~'æ!1©À;H4[Q_n@@`MȊÉ@:´œT^ý?'œÅ+	¿¨*Àüg£@‡0ž-}@!¯Påö"¿Ñ{%û'2¿çqÊÛ[¿è½*BsÂð¿å½Ž€á¼É¿ã1?=,±9¿ã`Æu(AGNRDG3FGL J1325.4-4301Cen A?ïùíŠe&Ô?B$·Á¯Næ?HIÕéç¨?B$·Á¯Næ?íí¢©HõN?¶Á‡™UÁ?°'ê´Ün•?¶Á‡™UÁ?î‰BÖ-7Š?ËâM.àR?§kÒ œ#T?ËâM.àR?î'ñ.«å?›fÍTâ#"?¯àë]s³?›fÍTâ#"?ïèyŒÅ?j…"\ìw?g†sws
ƒ?j…"\ìw?å4œbÝÖñ?Ò¶QIÒ:?ՖÇ:DR?Ò¶QIÒ:?î*§zûW? âkµÿ­?­UˆTš-‹? âkµÿ­?à¬Î}æØ?Æ0ǞÉ?Þ¦cÃ2P?Æ0ǞÉAGN4FGL J1325.6-0227?ꊤX&v@M¤Ù¾L×IÀ;$­‹¾åƒÀ<¡Š¯@ q‡^Ù8?ýªHiü?йܚ )×?րB¸â4@Á	š³u
@,DeN¿ïþ"ƒÕâö?ïüA™þCg?èFp¢¿ÖµÏÅ¥'¿åˆqy‹¿ï²!…‹ÅœAGNbll1RXS J132542.1-022800?ïñXa.ÝÓ?U½ZÊîÿ'?]O="«*?U½ZÊîÿ'?ïq]Õ%A?™€1¦º×?'ÔEWœæ?™€1¦º×?ïfÄɄ?ƒÒ€m´?ˆ¦z™rÝ?ƒÒ€m´?îï¤$"f#?ˆƒýj'¢?¡½·¹Ï?ˆƒýj'¢?ïêižæEÖ?aJÞ"?e–aIÔ±ß?aJÞ"?ƩzÁ?³EÈÇӕs?§D£˜×ïï?³EÈÇӕs?ïHÅM?"9Œ
 ï¨?–çB&½šZ?"9Œ
 ï¨?ì,àj'Tò?¬/,{N¤?¾˜ü®ÅXm?¬/,{N¤AGN4FGL J1326.1+1232?æ¿í"O,°@RRwÄ\»ÃÀ;p`B_öáÀ<ÁîqbBë@ ŽG¯—í?ößùµc#¼?⧻Ðüv?×k…òž?ù!¨¬\ý@]cIP€÷?ïé`p¾.¿­Æñv–¿ê˜¶zzða?Àe­™UÑï¿Ó
Ÿk?¿¿ðAGNbllLEDA 1410672?ïòÑhà6?V@gëD¼?[\ºÌµG?V@gëD¼?ïܧï%oÚ?…ú_'£ ?q¬ŽDRø?…ú_'£ ?ï'yO!P]?…k?•Ìmr?‹¡¬-]à?…k?•Ìmr?ïñGywvj?HX<NŠ8?]qíW;?HX<NŠ8?ïçpúµ?o.Nφ¬?hÿÖ©3Y?o.Nφ¬?ï‹þ"é~?a¶Ù*?z!¤Øw?a¶Ù*?ïSd'oa?'g|¸y?•"oÒÙ}Ì?'g|¸y?ïÍ(_D´?rL_=v?ykÐI¸<"?rL_=vAGN4FGL J1326.7-0503?Ï?TeD@LXÅCk›À;ÞÈè;¾À<×ÁЈg@"æt™Z­?ù2Æ[™ƒÊ?××Õ^Á¬]?´ìU~6¼«?Ԟ$ƒBM?ÿŽÞëuj¿äÁ@ýv8¿â¿Ýѿ恽¥œà¿ËbFÇÇÄ¿³ØDЩ*¿ÔLw½PØáAGNfsrqTXS 1324-047?ïþÃà—´?ý"w{Ñ?#ÁóÛa#9?ý"w{Ñ?ïòÕY°—Ú?^(»XƒÁ??ZUL€"»˜?^(»XƒÁ??ïòŠ³;šû?^ªBfçŸ?Zê™Z[4?^ªBfçŸ?ïýÛjêÅ?%8$%4Ý?1$­©Y÷¶?%8$%4Ý?ïÿC÷Å?ƒØ;•=t?"m¢?ƒØ;•=t?ï¿X 6©?"^侐[ô?€)÷øƒ	¹?"^侐[ô?ïò4·†ƒV?k¯:é&ž÷?[–',²Ãf?k¯:é&ž÷?ïðךŸíµ?]ëeûæX?^PÊÞa%?]ëeûæXAGN4FGL J1326.8-5256?ì´óʒŠÝ@#ÀL‹ÉÍÀ8"¶»éÀ;\hÑz±w@¡×sï»å@mŠaî1¡?©9è?U;­?Á ãd鹘@ÂÍáŸÂ©@ЯE¨UÊ?ãýߔO­½¿ß*ø…«¿â\¾™XV¿äsY(B¿é€ÞLQk¿ì5Þ>XˆAGNbll3FGL J1326.6-5256PMN J1326-5256?ïïÅY½?Yå¥@Þ?`ñ:«ÿ£?Yå¥@Þ?ïÍÝËo!?Š9«Ûø?y51¤a?Š9«Ûø?^Ƃ?ŠJL. µ?Žè`kY?ŠJL. µ?ïüÅ=a_k?(8%NÊ&?9ÖÑ¥Åé?(8%NÊ&?ïÅÙZ´Ò?t7p)<Ë?}S	ãfÁ?t7p)<Ë?íÿ.질›?¹Üák5?°ˆšÃ»+?¹Üák5?îoºÐ|k?ŸÏÈbjÔ?©Rþˆ9S?ŸÏÈbjÔ?ïôÐÍô{N?FÐpi‡Ý.?V^cóMt½?FÐpi‡Ý.AGN4FGL J1326.9+2210¿ï½À"x¤@T"¯ÌáłÀ8à~֟´fÀ;ÌËQ¢Š@}YÏT;—@î,ëñ?§›¶Õ>¶I?¾L`RP/@]"Äm'º@¼]*}'¿Áç~~á–¿âYÏ^ø]õ¿æåÂ!M,¯¿æçÁz‰3¿éò¶ÁG³s¿æîè`Q#‰AGNfsrq3FGL J1326.8+2211B2 1324+22?ïëk8]>Ÿ?x~MÆ¥?d"Lj¤X¬?x~MÆ¥?ïꃆݪ@?vGŸƒjç€?e|xûÚ †?vGŸƒjç€?ïcß#Ӛ?Ž»qC7ƒ?""]=ZÅ?Ž»qC7ƒ?ïðC‰í?Iþ¢…³o‡?_xì0'?Iþ¢…³o‡?ïåZàÿ½C?t+XzíÀc?j¥9ü-?t+XzíÀc?ï"WóÜÜ?™w-ŸO°?‹*÷F?™w-ŸO°?ï"ҽ҉?Õ'"ÿjv?‹÷KSúù½?Õ'"ÿjv?ï½ô}üì6?m	`ú]?€'àw&
¬?m	`ú]AGN4FGL J1327.8+2522¿ãì%²ìüÃ@TjGG"#À;¢
6Ih)À<ÜS'ˆ@!S `Q®?÷_›ªcì?Ú±ÜÜdok?Äß	$ìÉl?æè$¬‡²ç@ßbݚÐP¿åJ›ÏÔ¿
¿ïÔ~ýŒ`?ì?©-‹S†¿ß7ÀÜ~œ?"?QyšJÄ¿ãX^èm½AGNbll3FGL J1327.9+2524NVSS J132758+252750?ïú¤?©§ó?A²ªáçMn?EoîèË)?A²ªáçMn?ïõÃg.žŠ?^avz@ë?Ty1<f?^avz@ë?ïÖ©÷Ø
»?s¾(i]–#?t«
j–?s¾(i]–#?ïúÒh1 ?4½ý=Gå«?D¶^Zƒ 2?4½ý=Gå«?ïöŒÚT±?TN¹Y?SÊåûŸ®"?TN¹Y?ïÇbìª\?ŠÀǐ4Üz?|N‰ÿ‰iÌ?ŠÀǐ4Üz?ï©yoœ^à?†háäã¤=?…¡¤#7	?†háäã¤=?ïõ&õGÉ?QÁ}Æ7†?U³ÐråÍê?QÁ}Æ7†AGN4FGL J1328.5-4727?¤4çr¨YŸ@-ã
£3vÀ9tµÙk@ÁÀ;ÀŒŸ5@ áWÕ©ë ?ÿù6Òúä7?µc`øh\
?…³'Eæ?Üój:±VÐ@Σü¿è8ÅÖՏ?îAdÿ‰¯¿â]"Ð_¿áPj¡3–Û¿Û®ˆ^]ÙO¿ØVÇaþͦAGNbll3FGL J1328.5-47282MASS J13284063-4727496?ïý­ì=x?&6þ]C»z?2—^žÎd5?&6þ]C»z?ïçœ÷	?vúFv<¸d?hc;9?vúFv<¸d?ïï½Am‡?`¦Â·ù¿?`B¾Ñ—xá?`¦Â·ù¿?ïòŸ~ØD?IRØè&?ZÁý§A?IRØè&?ï÷1Â<G{?N×ävÞ±P?Qœ{vòéU?N×ävÞ±P?ïm¶j? ™KΝx?'OÉ*¦¨¾? ™KΝx?ï×Z%K¥+?{˜X¤xo#?tRígëÚV?{˜X¤xo#?ïÒ$š¿"?l¦V
4¡œ?ví²œ\.
?l¦V
4¡œAGN4FGL J1328.6+1145?ËÕí4×@R¯_Ô{îÀ;q3JEžÀ<¶èÒ¼ÐÖ@"&6oÓ¢?÷÷'#'?ÔÖNád‰l?ÇðZpŽÞU?ôÏsÀÁü@©_àˆ¿Â¸G"£é)¿Õ¿¯'ä÷;?Àˆ]¥¢'¿Þ=—$Ê9Ê¿"uUËFò¿ØY9W9£AGNbll2E 1326.1+1200?ïûþ;Ðï?4
û[
#?@ÓDöS(?4
û[
#?ïízkÎQª?jå‹17_²?b…"ìö&Ò?jå‹17_²?ïã|©É½y?ežƒzQ·y?lƒVi¾ó?ežƒzQ·y?ïúH<s'Ž?4u8[Éi?Fß
O­×?4u8[Éi?ïûa¶˜?<,b¤%4?CÂxlçÄÌ?<,b¤%4?ï¢ÐÕE`?š/bëøm?‡Kʲ*?š/bëøm?ïÏ
H›G?z†o­yUÅ?xy{Ý4¡?z†o­yUÅ?ïêK̘Z»?\åXÇé­?e´3b%ä"?\åXÇé­AGN4FGL J1329.0-5607?îh¬º'>Š@y bvÞÀ7ÛjUß/¦À;ßTŽÍŽ@ÆCß}Ôl@Ì=s(? ;~.ˆB?½±•¹»"*@STâ°cà@º•¼?`é¿Æëðÿ\+¿áŽ›¤5Ôοå‰AAé¯\¿å¤º|h¿ëË7×âr¿åÀ~SÂöAGNbll3FGL J1328.9-5607PMN J1329-5608?ïñ½£uKÃ?Y\§½4`?\"¸ÿjúº?Y\§½4`?ï¤iü?xˆ?—ß©Þ"Ò?†å€ì²Aò?—ß©Þ"Ò?¬È—Ö?›G«‡¥Ò?¥u3v'œ?›G«‡¥Ò?ïýw<LŒv?(^üÎ*?4Fž.5?(^üÎ*?ïèú\tl†?^ª™ú›Õ?g£rÖJF?^ª™ú›Õ?íÎéBàa?ÀÙ¡–""?³'ˆ¶Äãú?ÀÙ¡–""?îºEŽw?œß+]`"?¤[¯ŠcŒ?œß+]`"?ïò±;²ï½?P×ôPzèé?Z‰TU%?P×ôPzèéAGN4FGL J1329.4-0530?íü·Øì7C@LçáüúÀ:¯'m-*À<P*º¾­O@§/¬@ti
à"S?ÉAV÷Þsh?Û£Ñ@yí­@ö¤^ïy ?ý¾£»º¿ï6¯õ%±j?ïæC_¿Û1W{fþ'¿ä'–NÜÝ¿ëFQˆˆÐ¿ïÿŒÝÉtSAGNbcu3FGL J1329.1-0536HE 1326-0516?íè¢ÍŽ­q?²ôžÿEV2?°ºé'@¹ø?²ôžÿEV2?餣xô;?Âuç½íZ?Émr/¿?Âuç½íZ?ìÕ^‰MF/?¡†…²j5?¹U·Mœ‡?¡†…²j5?ëmQŒ1§? s?)ðñ?ÂJ¹Ï;‰e? s?)ðñ?ç/`×¹Ã?ÂÕ²½(?Ñ¡Í>PŒy?ÂÕ²½(?Úc+bH8?Ð3"»ªÕE?âÿNjNÛä?Ð3"»ªÕE?æ:)+ÈZÍ?¶BÜâÂÎ?Ӌ­¨oJf?¶BÜâÂÎ?ÖÇ	¾?¶ñ§æ
'?äœ{qv¡?¶ñ§æ
'MIXED4FGL J1330.2-7003¿©ÉbªùÀÀ#éêÀ8±òAÑ[¨À;Ž¯­Uk@®b¬©@Ĥúö«Ã?¨VsÕå¡?ÂéËÎ|z@€èÈ«ÕÜ@ÁÝFl è?ÃÌàÃÏ£¿á§@¬m‡¿æ³˜H`¿棖b'$¿é,Ân¤ù¿ï÷`Ÿ'".AGNbcu3FGL J1330.1-7002PKS 1326-697?ïò¸Sez%?cÝùj£ ?ZXûRFù?cÝùj£ ?ïá-qÓ,?€Ö?nҍ÷:Ò?€Ö?ï¹!3¶?'/ÁI›n?¾÷¹ÂÔZ?'/ÁI›n?ïÿi nÏ/?…×e&?Ûðò­«'?…×e&?ïÒI0±?t‡Ð²u3º?vÛu‰Õcm?t‡Ð²u3º?ïgtÐ%`¦?£™€³ÞX)?"eûSë1?£™€³ÞX)?ïHnýŸäž?'úÑk7É?–ò Q*ÖH?'úÑk7É?ïýû~&>?&¹ÎÙKà?0$(Pâ*?&¹ÎÙKàAGN4FGL J1330.2+7002?Ó›
÷™™@G\xB0üøÀ:S¯Ã§ŠÀ<µ"Î~}´@BÊáæ'?þ2‡V ö…?·ê"ßph?°Ý'ýuâ?ø^–ÞÔ6N@
ÂÚq{x¿çéƽ¿пÞ'</Ü¿à	¦ý…Qc¿ÚÔ¯DP¼Ü¿â{Ó {‹¿Ýx"á{°{AGNbll3FGL J1330.6+7002NVSS J133025+700141?ïÿ4+^[3?
À—¡0?z—ß•JÈ?
À—¡0?ï÷–Ôº¤N?P"%ù®Ñ?PÒV^¼dÿ?P"%ù®Ñ?ïù0[J?S>Ô~(nC?K‡=öf#?S>Ô~(nC?ïù\³‰Z?1¬ZŽ$"W?Jøà}r?1¬ZŽ$"W?ïþÖÜèp9?5µ#)®å?"'3ÑQÊ?5µ#)®å?ï܉ÚΆû?tˆÔ@±»l?q»Of©?tˆÔ@±»l?ïù8B¢Î?bÁÏbe:@?K¿ï™½?bÁÏbe:@?ïí©s¬J ?P¯YbA,?bVŒ—7C?P¯YbA,AGN4FGL J1330.3+4441?á%˜Ýâ@Q²–»˜ÇãÀ:qy¶ViÀ<©-óXQÑ@`;€^µ?þ˜DЩ*?¶ÿ{?Áh§HÙ¸™?þTuˆBYA@u>Òx³E¿ÝG"Ô@_¿ØEL»D&¿Ü⛠ÚÖ{¿àF@V1dý¿âù|"MÀ¿ïþËê'QAGNbll3FGL J1330.0+44371RXS J133021.4+444117?ïúÝ/+ÍÊ?9d€öýÛ?D‹CöϏ7?9d€öýÛ?ïìƒ`ó	ø?dN,{¤?c|žåæ?dN,{¤?ïåÜù?Çk?lYèìJý?j# œ,ó?lYèìJý?ï"÷5Ô?jþY#í þ?‹99û?jþY#í þ?ïÝYÙ©îÀ?l—[€ù‰?qS$ÙSó?l—[€ù‰?ï´xm$¼?…Àœr$?'áä­²^ñ?…Àœr$?ï¼-U¬7Š?»tщX-?€ôªˆë{®?»tщX-?îF»:Ôe?'8¸]s?«"LQ¸?'8¸]sAGN4FGL J1330.4+3157¿át[Ȏà¿@TêòRÀ;q–EQCÀ<°0Š‡@>u–8Ê@A&ÜÛ±?ÎÓʗé@K?Ò÷ ¥U@R]šåÉô@ÿTWÆ™?á拺³Å•¿»Ÿß?&l·¿éÓÛ·lé¿ßâWcJ¶¿ïÿa_3¿ÞP·þ^•7AGNbllMG2 J132953+3153?ï´+J?'>ù"Ýf?'øºê¶½x?'>ù"Ýf?ïZÆ/NÍ?Ÿk§Ov?"§:n?Ÿk§Ov?ï
x¹qŸ?'&›.Ëî¡?ž°èÊí9?'&›.Ëî¡?î›tÅÏ­}?‡B£Kp­?¦H³¡MZ5?‡B£Kp­?î²Jµ°Ño?¥!xo¯8³?¤ÛT¤òé?¥!xo¯8³?녮°Q0?ĆB•·óÞ?ÁéGÑ>»@?ĆB•·óÞ?í(-T2B"?£ù²Éknc?¶¾•^mëã?£ù²Éknc?æX&ñl¥?´DeÕÇÈ+?ÓO²&´þ?´DeÕÇÈ+AGN4FGL J1330.7+5200¿ãÊ¥à`@P½çXÀ:*q?|ÌÀ<€ç"øoé@–A»6Lm@'"4H?·ª4??¡±…c°?çsqF"9@ùP¢"пæ	—Xv¹›¿å	Ý.Cà*¿åC‡sý'Þ¿ç•žvx,¿å'×="
9¿ïùía—ʍAGNbcu3FGL J1330.9+520187GB 132842.6+521750?ïþV®H¹h?Æ&åõ€?*•	'º%?Æ&åõ€?ïö5Íþa?XA)Á?Sٔ'Š©?XA)Á?ïó²¥õ.?\,E(4CØ?X›Ñãõ?\,E(4CØ?ïîâ¯&?MWçÁ2é¾?aøêFŒ)º?MWçÁ2é¾?ïýñ&À«y?#ùÝúY^¢?0vË&Îåw?#ùÝúY^¢?ïàãX¡	?o¤ì8ðÝÞ?o§V¡Çm?o¤ì8ðÝÞ?ïñuø:ö?f,Jê<§Ú?]Á–—Ôñ?f,Jê<§Ú?ï®{e?sÍäî
mð?"`!Bbؕ?sÍäî
mðAGN4FGL J1330.7+2933?êš{ÇÕ@T@ò@úœÀ:'ßBñÀ<…0¹o¬@Êiïۛ@›Û ¥&–?ÆšÍ Y¼µ?ÑÃZб@œT\È@H‡RŽm?ìs€àæ	_¿Õ]ê–â/5¿åÑu=™¾ƒ¿ìTR½'M¿íÞæÀ=ó+?åYã¡$¨VAGNbcuFIRST J133101.8+293216?ïç.)€yY?'5i}9j?hÑÖ£B–O?'5i}9j?ïõ.%ŠÜ›?b)sDYñð?U£µ]¹©b?b)sDYñð?ïWS¸R±?‰çZïD-ó?•ˆõ©Ý+?‰çZïD-ó?ï슻Árã?O­0ÿËàB?cuDI‹Ý??O­0ÿËàB?ïíôºôÕ?b,U
™È?bçI*²ƒ?b,U
™È?ïÔÉýÔF?ƒ3ô—u¶¾?uþä9%h?ƒ3ô—u¶¾?î_½…ßd?œ›2Ú¨?ª.¥TÈ?œ›2Ú¨?ï•mÖOàñ?{lN^'Ž?Š¤ŠZÙ·¹?{lN^'ŽAGN4FGL J1331.0+5653?æ\h2ÃT@M´k&¿‡jÀ;Zw'ÔáÀ<ïcáPèP@ ùŸõÿ 1?öûUvT?ØB·ÀK41?ÒFŠþÌ#?õb¥ç…¶?øj¶ü¿â°›ÿ$Ô¿ê[a .Q¿çp5½Q.Ç?ªÁdÂUD¿ßZ_U¿ÚƒT]ÐAGNbll3FGL J1330.4+5641RX J1331.0+5655?ïûôÚªRq?2sJøÆ€?@," 1cî?2sJøÆ€?ïíÞ)ìb"?c
¥3wo?b!Õç¢kó?c
¥3wo?ïÌ'Äò?s¾Ñ›@sE?yìs‡<nù?s¾Ñ›@sE?ï×:ÞgÖ?] *OYc"?tb´fÑ%?] *OYc"?ïýsü¯œ?09º'õC{?4`|'?09º'õC{?ï»úJŇD?'°lò' $?mOþä?'°lò' $?ïÒă'<Z?N'o]'L?v¾sðöù?N'o]'L?ïN·ÃÛs?‡g‰VIq?–)äõ­?‡g‰VIqAGN4FGL J1331.2-1325¿î½š8a+¥@H'M3H,À9™X¸'úÀ;ŽŒ3‰M@4@#‡@èŠÛ´ï?Ã>êáà°/?Í&ö9ÔA@ PxË@4j­óò¿ç¬h=Öû$?À‰ßgY+¿æ ¤_ñ,S¿ë`ö í¦¿ã°W¡&«»¿ïÿþøþ"AGNbll3FGL J1331.1-1328PMN J1331-1326?ï÷Jø`¼?LªÑß¿?Qj-9ˆ?LªÑß¿?ïëü·dõg?dåEƒ³¤k?dHÔÄÌ?dåEƒ³¤k?ï'×mº˜˜?†DtPõû?J$¢‡åù?†DtPõû?ïâù¸ìž?TPÓÿ‡dW?mGÈ6ª'?TPÓÿ‡dW?ïÝ3¢Câ-?r–›tO‡!?qf.×/±†?r–›tO‡!?גּð¥"?‡ì]ˎ7?"ÓCÚ+wV?‡ì]ˎ7?í}eœ?¦ã»ëlå?·ÄÒ>¡?¦ã»ëlå?ï¤W5?þ˜†P?ž‹u!fÃ^?þ˜†PAGN4FGL J1331.6+1711¿èõ½B¯ì±@SEbàŸèÀ:@óÖ&À<ptšÐ$@-…àT>@Á]}‰˜›?¹<ÀO»Õ?Æí|Õ¡?Âi;,ü¸@R:«økâ¿Ý«$[¾¿æ1L©%þ—¿áëâ—°¿åTÍ·®X¿åÚ;€ÎÜ¿Òg'áC§JAGNbll3FGL J1331.5+1711TXS 1329+174?ïü_À¨Ž?6SŸrc–?=ÿBŔK?6SŸrc–?ïðÇ·ÓÛ#?cRò.áµ?^pÖ»YÑ?cRò.áµ?ïéǗ®³?hDÍÓÊ¥P?fé8}?hDÍÓÊ¥P?ï÷(À_ù\?>A
OŸ[t?Q®~ÏZ?>A
OŸ[t?ïøÜ°€Í?KŒ<•dP?Mˆ}ÂXs?KŒ<•dP?ﺅ%Ýùà?‡ÇY"f?^¶{Êú+?‡ÇY"f?ïÜïôë?w£—%ùGU?qˆqc§'©?w£—%ùGU?ïØ$pf‰;?e¿"¾â?síÇÛ)¾Œ?e¿"¾âAGN4FGL J1331.7-0343?¢?UKÿ
v@LÓ;÷'À:]òœj.rÀ<Õ¤ãc@¾k[m¹í?ùæ(S`'?ì1d™ˆ?æB^
ÒQ?þÛÐ@Ô@T@¹Ù€?åðg¦ØF~¿çQHÇïî:¿ã&ØaU…n¿ïÿèã«6¿¸š¬È®¿î:
BâMAGNfsrqPKS 1328-034?ïü£Úî¬#?^#bµÍü?:á*$7?^#bµÍü?ïîŒbރ?eC×\»?asç…Ä%b?eC×\»?î'xú#u?æLý>­?§Øpa?t°?æLý>­?ïûqUå?7UÎZÞ7½?Cæ<D\Ûã?7UÎZÞ7½?ïú
î¥H?aÜRIóL?GÔG¾sÄ?aÜRIóL?ï¦ðŠŸ´C?"Àû Æñ?†CÝJT7?"Àû Æñ?íÑnzºŽå?¢ËA5Ä ð?±tŒ)½•W?¢ËA5Ä ð?ïî	š!m¨?`FCšÚB?aöe¯×¨"?`FCšÚBAGN4FGL J1331.7-0647?ïÿûäE@KY†üÞãPÀ;ÂHåL À<žw{@áqF>RÌ?ü™ƒyœ¤?Ïm"ÝzÅ?ÓW,u©Ð@»
,©¬@6ŒØ–¸¿Ë»±\"?ïø €´ã¿ËÊ+éÔ¿à›¾'1H"¿æW9''¦¹¿á¹
"BËAGNbcuNVSS J133146-064632?ïô1Ôt?}mî8	K?WœVÄO(F?}mî8	K?í*Ìn?Œ¥âM²F?ŒžD¼,'?Œ¥âM²F?ï§0ºPj?pÿ¦Ñ¬?†3Ñv|I'?pÿ¦Ñ¬?ï5>F"?yˆFÒµÁ?™\x8çKU?yˆFÒµÁ?ïïU.Ê\Ÿ?WæC¹cɉ?`ªÐóªá…?WæC¹cɉ?î52"ŒK?´È|F|°?¬®ìÕmZ?´È|F|°?ï(G"îp?"r)9˂ê?š÷çù?"r)9˂ê?샌ÊS? ~îÆ$E?»ãŸa¯g? ~îÆ$EAGN4FGL J1332.0-0509?ãJhH`8q@Läy'¼VÀ8¯ ÄÀ;'ŒÂÂ#@	"'›Ø@&Ð& û? Áø»ñÚ?Å[ôœî¹@ †/Y‰ß@»û¢£-—¿ÓéŒÁDŽ¿á•"Ì'úò¿ç–ªÁµ£¿êqü!#;C¿èÜ"¤?¿ïÿ±Æ·	AGNfsrq3FGL J1332.0-0508PKS 1329-049?ïèèIØw?k?óÓ|_f?gàùàA?k?óÓ|_f?ïßù'jºÎ?"c'îê?p7W±?"c'îê?îöYa`y?˜®»› O®? šiì5{k?˜®»› O®?ïþíñúH?%œ±kÖ¬Õ?.'8Ûý?%œ±kÖ¬Õ?ïJEAŽÑÑ?•#®ëä‹?–·WÕýá?•#®ëä‹?ïƒõ­ìŒÜ?£É*é© ?"wY,?£É*é© ?îœèæUV?ŸŸ¶ã-A?¦>1qšª™?ŸŸ¶ã-A?ïô!¤YTõ?PÀ[l«)?W¼·¾	Eè?PÀ[l«)AGN4FGL J1332.2+4722¿í•Ò¢y½@Q篷éÀ:]N[­¥ÀÀ<tZ5Ö{¢@E–hâ˜@Å1Àll:?À±µY¾D?²†¯‡µ#?ïOo^²'å@
$¤¥p;?ï¿àÀŸ—à¿ãiWaæ¤å¿é-h]â^Y¿æ°<g™í¿ëñ§½s¾i¿ïí…èÜÎAGNfsrq3FGL J1331.8+4718B3 1330+476?ïûóù·f‰?I-ƒŽ^N?@0S#Ó?I-ƒŽ^N?ïö•Îça×?VÆ!7S0?RÔaÆ'n?VÆ!7S0?ïéÜÊñ«T?fÌ»±NȌ?f#5"üƒ?fÌ»±NȌ?ïîz8ýÍ?JÎ%7S³?a…ñË!º…?JÎ%7S³?ï÷D]Z¬§?W#n#ÞÿB?QwE!kaW?W#n#ÞÿB?ïÛ$‹GÛ?túͦ
ˆ»?rmºpdN,?túͦ
ˆ»?ïê÷›5-½?m ¼å®X?ed¡–ó_?m ¼å®X?ï½ý¸Œ?m}ÔëIýŠ?€¾ÀŒÐòò?m}ÔëIýŠAGN4FGL J1332.6-1256¿ãnjõI÷@HYµà÷üüÀ8ݜþ¨èÀ;.
—~6@†/8§¼G@8"üS£? øÙßɘ?ÀÄEª.<S@ØFèòA@õxèt¿ÕH­ûŸH¿â׌™¿æ=é¿æЖP8ýx¿éL!`ø¾B¿ì
Gahz¾AGNfsrq3FGL J1332.6-1256PMN J1332-1256?ïð_XL"¦?\˜&o#F?_AO£Oԕ?\˜&o#F?ïÞDk6QB?yþ¢\1Á[?pÝÊ`êí?yþ¢\1Á[?ïOÄø±ÆÑ?"/[bQY?–`ð¦]Ý?"/[bQY?ïó|˜›±'?O}õ^'þ?YÎô—Þƒ?O}õ^'þ?ïyS_g]v?‹Þ'V@¼?Õ"«W1?‹Þ'V@¼?ïk‹‡eÃ?¢Quœÿÿ?'Žo	9?¢Quœÿÿ?îzÐÚè2H? ÷}ú|"m?¨RòS4©'? ÷}ú|"m?ï|éÀM|?ƒÈÃÇ£>Ê?bÇöNPp?ƒÈÃÇ£>ÊAGN4FGL J1333.0-6626?æl.Šé
ÜÀ9æRlÀ9åüágŽ…À;|Ëëü<ý@<r‰à>@9Eßaô?Б} <5?Òb÷{Ìÿø@3.`e›e@QøV¾R·¿· o Ê$ý?ëñ_ˆ{º¿çGQÞD‰¿è³¾smµæ¿ïÿ틉5ž¿ä9óEAGNbcuAT20G J133254-662826?ïº-žµ?³\L
‹%?{4¤<Ì?³\L
‹%?r⠟?'°¹|Öä?ŽÙ#6)Ìq?'°¹|Öä?îð¯hkâ?"G1Yù¢l? õ	|·}ß?"G1Yù¢l?ï^"IÚzÇ?u¥")É?"-–ÍG­$?u¥")É?ïŒM³½[?EI£}?Œì"
=#?EI£}?ìÂæðöˆï?«íÑv¢?¹èÈxK¸ˆ?«íÑv¢?é°Â·òö?¯ö,Ȅ?É<÷­ 4(?¯ö,Ȅ?ê·%b)É?«‡42ÔÁø?Å#jw[ðÛ?«‡42ÔÁøAGN4FGL J1333.2+2725?ëϾÕ@T,¯¢ðZqÀ9åkÅKÀ<ƒˆ×@yÄqßk`@/${	‹š?³5ëId¢í?­/)ä*—?öôLfàà@
"ÞCÿ ÐU ùè¿ãX˜GŠM¿äH3
‡¶¿äbYDzä¿ç#…uö&b¿æz˜í¢/jAGNfsrq3FGL J1332.8+2723MG2 J133305+2725?ïýº!ñ¹¹?'0´IÆ>è?2.òv÷xˆ?'0´IÆ>è?ïõaQ1S"?^Ú÷Vg?U=]tŠà?^Ú÷Vg?ïï…,Ð?fJ)Ša*?`èzñlx&?fJ)Ša*?ïéÏ-M–?Pïê²³•r?f0çìy­?Pïê²³•r?ïù¯öA)/?AìiìtN?I@%ï_q?AìiìtN?ïؒ¨0,»?ùGö¬ù­?s¶«æ‰ÊŒ?ùGö¬ù­?ïÑü»Á¦m?d@gb?w¢]µ?d@gb?5+9®f?mùË׆›?€Úµ*µ.w?mùË׆›AGN4FGL J1333.7+5056?֛F‡@P7Ù+à‹À9QpXW¯êÀ<&€Aÿ@Ž5deÛ&@oZµ?©Šނ›•?¶ðBrÁ=¢@äLæb @QúÝv?ßÝE€gÄ_¿âïÕ¿ä•`ß鵿äl¥¡·¿éJS
iŽ¿ïüÒf(SAGNfsrq3FGL J1333.7+5057CLASS J1333+5057?ïûj·ƒåR?7˜ÕÎÈ+?BU!ÍÈ@w?7˜ÕÎÈ+?ïõE¡õ³¡?`ù^ ©>6?Ut»ÄáÎÁ?`ù^ ©>6?ïß)W
?j9h ©Ü?pkT_Z—?j9h ©Ü?ïýÛÆmjÅ?½™/xd?1!Ët—eA?½™/xd?ïú~é¿÷§??\ã™	¬G?FY,©‹??\ã™	¬G?ïÝÚahƒU?sD¹£_W?qÏ*)Ñ?sD¹£_W?WFÁc?†Çî^Ãb?ˆPj!›S?†Çî^Ãb?ïûxâw'?4f©¬0%?Buî¾Xi?4f©¬0%AGN4FGL J1334.1-3521?¸Ú°æl@:´óý">6À;†qž¨ÍÀ<µ—îáË@",Ò£üI?û e›eK´?ÇÜìš"ì?{øVñÜÚ??¸=¾./?üKÛÙ=§¿îGø½Ÿ¤?¬ÜUÖÌ?ïçB.x¹O¿º‰#ªª
/¿ê<Œ¾÷Y?Ï1úcˆænAGNbcuPKS 1331-350?ïû•Õ"Çx?<m#ê½?A¨¨ùø'?<m#ê½?ïðn™T"?`é+wZ?^ý"_cXc?`é+wZ?ïÊc¿Ý?uïF¯qß?zÎ "»Ù8?uïF¯qß?ïç®ÿ?ZN9¨|
R?hòÌ¡?ZN9¨|
R?ïö'M›]?N-Áû"?S±e3ÿ•†?N-Áû"?ïÇH·\€½?€Ý¯x÷E?|[¤Lð-ƒ?€Ý¯x÷E?﬉rã€?…\ÄOD	?"ûª&Wù?…\ÄOD	?ïÉKü‹^÷?r~›£Io¯?{ZË~v?r~›£Io¯AGN4FGL J1334.5+5634¿ÔŸ/z0@MÈà"'À;J&˜=™À<¾2‰}Ã@ÅSÅ$ù@÷çbzH›?ÃJÕ¦»?¿ b3Ѿ¤?ܦÆ0<‰@£úü5>¿î3(¶ØnÁ?ï®þ`¿¿çêUp
¿ã½¢W®<¿¿êøýâïN?Üá­å+}AGNfsrqTXS 1332+567?ïù¡<XÔ`?Qbh˜OÚ?I{
«V½©?Qbh˜OÚ?ïôG4>mp?Xkb?Wq—0®¢?Xkb?ïºú˜?¯÷?{`¬äâ.¿?AY÷û>?{`¬äâ.¿?ïîÛ×ùóï?Jœ¶t?a$(ii?Jœ¶t?ïã½S)•?jìãö»"å?léBl=Ã>?jìãö»"å?ïÌëÁ14?y'FNñè)?yŠ)?y'FNñè)?ïuåî?ŽcÁƒ^?¹âžü"?ŽcÁƒ^?ï{&º²v"?'ï4¶é?›(°eš?'ï4¶éAGN4FGL J1335.3-2949?ïý9P'Ë@@
=¢ø½ìÀ:_ס<%JÀ<i'Où<—@ÏÄùÛ?ÿ@Íù¦J?º[ˆ'ßf?›'ù†-?átþªëQ@é
<€?î&üX«'À?ÓsºÂ‰'¿âþiȶe¿Òi7;«|Æ¿ån)¾ÀD©¿æ¾[ÏßAGNbll3FGL J1335.4-29491ES 1332-295?ïýéæÊ5)?"Òsƒâfð?0°Ë6ÝH|?"Òsƒâfð?ïðq5çy?a½BÙæ³?_"µä
ë?a½BÙæ³?ï÷¸¤)s?@=N<ã©2?PŽ·GeSq?@=N<ã©2?ïðBq®\ä?FT¥:,.ÿ?_{Ú?÷É?FT¥:,.ÿ?ïûÃNúº?5ymõÛÿ?@󃢻Ç?5ymõÛÿ?ïÎ18½?z罆æ;?xç1pD?z罆æ;?ïøË,Rˆ'?` ¦Ãî•Á?LÓOeËcO?` ¦Ãî•Á?ïÛ—0Cü?`+'áDwÚ?rp4Qà'??`+'áDwÚAGN4FGL J1336.2+2320¿ä܇ã8Éö@SÌs-õÑÀ;:ØC""À<ºoª²Æ'@½mç94ª?û.ʸöV3?ÓÖBAn	s?ͽ—»!ú?÷إ̭Ã@ۅ9D†?ë·Ç'
0Û¿ì=¥b$¸F¿ÍºÞæ¿Ç°j–vÏj¿ç€…@dž¿ïÿÀªšëAGNbll2MASS J13361219+2319581?ïû/"¤½?=G_sþÙ ?C—CšBuP?=G_sþÙ ?ïð‹Ÿäj?ji}Eč?_Ìè²x¼?ji}Eč?ïºÃ¾cÛû?á'#%†?Ot…'?á'#%†?ïΉ¼+?_.FH£?x»sþ*±?_.FH£?ïûrP™9f?A`À|?B6¼Ï±ˆ?A`À|?ï¿87 u?ŽqÜi·yŠ?€91ë´Ç?ŽqÜi·yŠ?ïš+õÒ)®?‰LHΓ?‰u•Ähs?‰LHΓ?ºþÍ?vN–_0ž?‰˜`@í?vN–_0žAGN4FGL J1336.2+2053¿æ"¼ÝìYÛ@SÿëJÀ:ã
æãÏHÀ<•¬Þð¼@¢3k½=c?þԓj«p?ÍÙ_m=p?´".›säS?ê–
ΐl@,.Œ…_?ﺌޠ3è¿äÜÃàj
¿á‡—¾V迼e®Ûu1/¿áƒ"Ê/c›¿ç×_f˜AGNbcuNVSS J133612+205102?ïùI™•×‡?YK"e¼Ã?Jٙ³ç)?YK"e¼Ã?ïðøð0?lØÒº°"*?^yTA+?lØÒº°"*?ïÂ3EŸø?'•Ðgc?~æ]!X<E?'•Ðgc?ïéï®×¢?LÏû
6âƒ?fë" Ý´?LÏû
6âƒ?ïû›Â=Ҟ?Eªã3²Õc?A÷«üŽë?Eªã3²Õc?ï³#WaÕw?Q{|RU?ƒ7*ãØX?Q{|RU?ï±³ÙXBÚ?ŠÆmJ ٖ?ƒ"	™É²?ŠÆmJ ٖ?ï½o–ÞÓ?p&¡˜Ù7º?€¤YN!4?p&¡˜Ù7ºAGN4FGL J1337.4+5502¿êo<dùîˆ@Nm©CZÈ£À:ôå‹àssÀ<¤ÝŸ'ç¦@_o̵@Æ"ï¾?ÃãŽe?•g³™ú"?Ñrd`ý›Í@
Íî¿›\¡õ*0¿æp@o[Øn¿î8¯6Y¿ÍÈ#à{Ö¿àAœbKό¿ïí…>˜ÂAGNfsrqS4 1335+55?ïÿ)ÈȨ?4ƒ'h?Æá…ïÆ£?4ƒ'h?ïø;Š›Ê?P_ÃU'Š?O×ÖkB¾?P_ÃU'Š?ïëåecËÆ?iO£å£Œz?dšxxJ?iO£å£Œz?ïþ'}ÁKå?­ln¥?&è"wŸ"+?­ln¥?ïÿ=Ecj?¸"IQLq?WOö¶e?¸"IQLq?ïà…¦È9?q°8â0ù?ozXû§¯?q°8â0ù?ïܦ\?wË_—ó°?q¬·ÿñGm?wË_—ó°?ï÷aû"K?G•'wNb?Q<
KÎ)­?G•'wNbAGN4FGL J1337.5-7802¿éQÉ5`"À.ÉÄüó0À:¾eò£ +À<jGW­eÿ@l/µÐ1@¬¸?wT?ÈÍvÀіá?¸]/ÛåÄ?ñtVéò?é&ƒZ?î48Ùeb¿éÄ×5›J¿å"åÕ²O¿ÐÓDá"é¿æŽBM'j¿ïÿ«Ÿ7=AGNbcuRX J1338.2-7801?ï÷-+hû?rŠÃ!?Q¥©±5ŠÛ?rŠÃ!?ï$i}-?£4€UÉâÂ?›}ÿ‹ñ"]?£4€UÉâÂ?ïÁXÃn1ê?ƒ,mó(Ñ?SžLV¦È?ƒ,mó(Ñ?î¾|}˜Ì?"¶ó$X§?¤¸5'¾F?"¶ó$X§?ïù8iß?V·ãfVH$?K‡ÇñÎM?V·ãfVH$?ëÙ¶è^ù‹?ÃÇÿCÓ¥•?À™$^"Ö?ÃÇÿCÓ¥•?ï¹Ãeùa´?…Çh"Ûw?&€Ÿ±?…Çh"Ûw?çÃDžü–$?°,›q¦"?ÐyvÂÓ·?°,›q¦"AGN4FGL J1337.6-1257?íj'ê2kì@H0W\gÓÀ8¼^ÑF¯À; *o?Rü@€|»@p…ÔÀ·?ªâ¹âÔú?Á·œäÒ¨@÷x‰|ì@;ñ®ƒ‹?ì赖Ob>¿ßI¼±K½¿åºß.Ï d¿æÉë	ζ¿çüQ¿æ4}¿ëãú !°AGNfsrq3FGL J1337.6-1257PKS 1335-127?ﻎÁd?²îÒö¦rÃ?_€œß&?²îÒö¦rÃ?ïÙÓsòÊ?ƒ¸´þÙ0?ssµˆ{M?ƒ¸´þÙ0?ïËÚÚ¼é?y÷*;Ž[®?z"^»3?y÷*;Ž[®?ïÓë+©ôR?\¹?¨ì°³?v
j;ƒöÜ?\¹?¨ì°³?ï÷I½ä&±?O#át¨¥•?Ql"`íî•?O#át¨¥•?ïk"9?¤ë\¾s¢ø?'ïl^øß?¤ë\¾s¢ø?ï'*¯M'a?Œ³Å¬×jß?‹µT3~Ÿ¨?Œ³Å¬×jß?îéOrëH?Š;/­¡÷'?¡kÒ*'w?Š;/­¡÷'AGN4FGL J1337.9-1956¿î}¿®2E@DÌsWæpãÀ:ó/p0ÄÀ<;+äŠX´@Œ·ÔCé@¶5¾þ­ð?̇À键£?¢(^Etm?ÕØÙJ‰'@
lš­•Ïà?튌Jü}•¿é¨USïk]¿çN'ÿú ÿÝEâb`Gh¿åšVÞ3&ž¿ðAGNbcuPMN J1337-1958?ïþìY¯ô¥?ì-lɑ'?!:d—(x?ì-lɑ'?ïõg»{Ë?XžÀRž'?U0ˆñ:G?XžÀRž'?ïôyWÀíW?KmÉ°n—?W
P ¯òÿ?KmÉ°n—?ïþ
¯Cû?Vs	"o"?/^—ËpNÅ?Vs	"o"?ïÿl½v K?9¬\›ÑÄ?hN'nÛd?9¬\›ÑÄ?ïÏçøˆx›?|$6¸È6Ò?x™gš™?|$6¸È6Ò?ïðW.B¼?lm~Ñü?_Q£…J5?lm~Ñü?ïöµK{Ôb?D†Ï$.uA?R•hdý%?D†Ï$.uAAGN4FGL J1338.0+6534¿ã"…;	@In¤"‰—ÄÀ:d¸ÄL0À<…Ö9ïæ@´`àÀu@!‹…ÚŸô?ã%Éé±?¿6Ü
,~¹?øôèû¼¾@
)Öð? °XÍÌ|¿æY	áÖZ¿æºl­¨DW¿ê"öÕ®¿ïÿµÝœþ©¿ïÿ‹Á>ÏAGNfsrq3FGL J1338.9+653287GB 133543.8+654752?ïüþ|×?-±­sØu;?8:3K€?-±­sØu;?ïô&ßׅQ?VeÖtDŽ?W²?þ~½Ï?VeÖtDŽ?ïé'UW™?Wvèº-œ?fØ«ä÷O?Wvèº-œ?ïÐzÁ½$8?`UáLxa?wŸ3ûÇÄ?`UáLxa?ïüDwð
?6%×±8š?=ßڞ¯¤?6%×±8š?ï×¥Îêù?rbýÇª?t-|"»‹?rbýÇª?ïæ¦Òxo?p1U܂+Ò?iïXõ-ùÁ?p1U܂+Ò?îë™É\?‰&¼r{a?¡Nb'ÓI?‰&¼r{aAGN4FGL J1338.9+1153¿àô#P<-ƒ@QÈ\|ؙÀ:»WYƒ)À<XEq
‰@òv`¯m@@uá;ÚÂ?³AwïzÌ¥¿–gڄÆMØ?䆼²£UÛ@ûû!ÉÔJ¿æÁáìï'¿Òƒ`½Z¿æy¶Vi¿Ýá‹5RÈ$¿Î†Ï'y꨿è'?
äAGNbll3FGL J1339.0+1153SDSS J133859.05+115316.7?ïþm9þ?$MjÖvÖÒ?),o妈ê?$MjÖvÖÒ?ïóô³4?aq¸!^?XšÕP?aq¸!^?ïñHl«Nù?o~Ø%!±?]o&(0¿F?o~Ø%!±?ïÿBÚx1?S+¸íŒO?¤ÇïÓ¬f?S+¸íŒO?ïþK¢¦ð?#u™¯"Ӂ?.»F±x4?#u™¯"Ӂ?ïÆ!軞Z?ˆ·±·¼}?|ï'"kD?ˆ·±·¼}?ïò 1?p|S¸Ï?[Õ¿¥GþÁ?p|S¸Ï?ïýåõxù¢?'?èM8¤2?0ÐU"¥n?'?èM8¤2AGN4FGL J1339.0-2400¿ê–NÃT@BËw[0À9përáÀ</;©#z@ÐÃ7LÈ[@÷3¨£ù?°k̬Ái—?®ý&¾%.?ýt,!Æú%@tn}·÷?äuÞÿT^¿âJiæM§S¿ãqø -à¿ãô±œ]™¿è~¶ôô3C¿çR¾éµ;AGNbcu3FGL J1338.6-2403PKS 1336-237?ïýî"ª?&dF.. C?3xŒîÂ?&dF.. C?ïô0Yu?]/‰ŒÀŸ?WáÑ÷Cë?]/‰ŒÀŸ?ïðnžÝêñ?cÍE˜è{?_"ÁÀ9?cÍE˜è{?ïùÌDf·D?6@JZ
z?HÎía¦×=?6@JZ
z?ïø—Çɾ?GJž>='Ã?M á&ŸÓ'?GJž>='Ã?ïÈ'*£S?Òy;­Žš?{ù¿
J¾a?Òy;­Žš?ïÞ»÷<?wF+Ñ=?pþ!è4í«?wF+Ñ=?ïðЀǡÑ?O½¨Áá?^^þk<þP?O½¨ÁáAGN4FGL J1339.1-2620¿Õ'ƹå@A¨hۋ¬qÀ:u\€3—À<o'OÐ!ì@_y';|-@RÑ84$?€*ä ©?¹LuN‹©A?öÈÝ•.@
'áG®{?ïJùùUÁÓ¿å½K_¤Ö9¿ápXô©¿âÙs8ÜÀ`¿äÅ"}c¿æŠD'HAGNfsrqPKS 1336-260?ïþ#½°‹_?Ž±žÛ¢å?-Ä(qäÍã?Ž±žÛ¢å?ïô³@•i?Y5w:/
	?V™Ëq¾i?Y5w:/
	?ï÷x¶0d]?U-'Õ­Ù?Q"€ú¶?U-'Õ­Ù?ïüŽT}A? æÕSP¤ž?;[Ÿ8>? æÕSP¤ž?ïþX%[?#wã¢5y?.:}~Tʀ?#wã¢5y?ï͸.§®?|¹HR€ˆ­?y#è·>é?|¹HR€ˆ­?ïø°WG?_Xoz-ºñ?M>£Ežc?_Xoz-ºñ?ïõßàкÃ?BAAÎ ä/?T@=×Ùʧ?BAAÎ ä/AGN4FGL J1339.9-0138?ïF\Np·‰@Mzj~ùÛ#À;=[XkÀ<ÜãèrDÁ@‹‹ØeÝ@ñ·D¥?їÆÆ"Ž ?åÀGƒLP;@Qͽ"©@ ß=è˜Û?ïõêgèF¦?ÜWžbP2¿âG~>œ¿å @LÜ'¿ïÿ¶>@£?ë\e[¤k…AGNfsrq3FGL J1339.8-0133PKS 1337-013?ï9'žV?˜mi§óÖ?˜Ü
Íí
?˜mi§óÖ?ï†{Øú"Á?œ\w÷ž·°?Ža	È:GÎ?œ\w÷ž·°?ëš0áÛbù?§ogÍáÎ?Á—<x't?§ogÍáÎ?r§^Ì?v¥ ¶?ŒÝ£]…?v¥ ¶?ï*௾Û.?žç¬eèÖÝ?š£ê$šG?žç¬eèÖÝ?íšolkÛh?¹«¢ìºº?³,"›WJD?¹«¢ìºº?ã:Ì&´Ÿ¯?·ö$ü7U?يg²–À¡?·ö$ü7U?ìڏ²ÝYÚ?¦}`&T±?¹+'jÌÿ,?¦}`&T±AGN4FGL J1340.0-1501?íaA¯*ƒ@G›¥ãSøÀ;XB 6mÀ<®Ö0ù@!j¼<ܪ:?Ûeºnü7?àcÞÌ©'^?îȐB@™½ÆŸŒ"@qëô…M‡¿îôŽŠïˆ?ïñ4?ø"z¿êì>ý–Ä'?²Ë;A
€5¿Ñ΂#Ü(4¿èMnGÜ7¤AGNbcuNVSS J134005-150314?ïߧRiÚ9?¥ŠîÂ&;å?p,Vê¯K1?¥ŠîÂ&;å?ïë?'-?pQØs³O?dúÀ4"Ûe?pQØs³O?ï™Uŕ‡"?}Ǧóp.?‰ªŽŒßDz?}Ǧóp.?ïñþŒ¯È§?N+4=?åå?\çâЎ?N+4=?åå?ïÂo¤ã?ƒàyW"ßP?~õH=Rg?ƒàyW"ßP?ﰝ͗?µ6SQ!?ƒûX–9%Ý?µ6SQ!?ï'ÆÎ}sk?ŠžBpžëÁ?NLYÃí_?ŠžBpžëÁ?ïí7ÑR˜~?aÏëoå+?bÈ.ª§ÑÈ?aÏëoå+AGN4FGL J1340.1+3857¿ëûîJ 
@R™çW"À;3
s†
À<°¦°ÙQ@@§;N
@>Ü~ñw§?ÌӒy>Û2?Áîj@æz?îuà÷üü@@躹¤Ò?ïÿȂeJˆ¿ä­v€d¿ë]Ä×5¿à °)¿é•ã+³ã¿ïßÓo~=AGNbcuNVSS J133849+385111?ïþB!º?+LêK̗?.«àº³¤A?+LêK̗?ïóËÇDzå?ið©j+ö´?Xhpä
?ið©j+ö´?áEˆS?4mîº?€G­>B?4mîº?ïëS<+ï?M$xV£ÃU?d¬Äë,º?M$xV£ÃU?ïüµpÛ»?>ú†ÓË?:T€°æìê?>ú†ÓË?ïÔB{5ç?wÁ»î£wA?uÞÂmû<–?wÁ»î£wA?ïKôµ˜e?'èɍª?–ibt]X?'èɍª?h.¬U?}qî€`în?×åþ£¾É?}qî€`înAGN4FGL J1340.4+6926¿íR̸k8@GŠpCßÀ;µ?ÇÀ<DZ«ß{@dlƒ¶ÙF@v†a®pÁ?̎	Ãx:N?ÂþgN˜¿?òMº°k@À"CÆÿ-?ïÚKäÚá¿jÓaL²Fu¿ë:ñ£EêÆ¿ÙÛˆü¿ïÿÿÊPË?ï½%?T©¦AGNbcuTXS 1339+696?ïþûU¡G8?$x Là? J¥Œý§k?$x Là?ïøýIÓo?M'ªƒ¥?MÀB̚E?M'ªƒ¥?ï°g$bœ?€c9~-"×?ƒæ6Úúcf?€c9~-"×?ïÿþ,#>ý.¹Zâ_?€r}&þ>ý.¹Zâ_?ïÿ=*?#‰/l;ÖÝ?ZÂj\•?#‰/l;ÖÝ?ïÞ}Æ¡±ã?r9'`¢—?pÁ¤(N`?r9'`¢—?ïa½JVmþ?'ïq´Å'g?"ÈV±Â¤8?'ïq´Å'g?ïþÅãyŒ‰?§Hû«"Å?#¡Çì?)?§Hû«"ÅAGN4FGL J1340.5+4409¿Æ¤vAzÊ@Q"¦ YŸÀ;•/§xÀ<©u¹À€Ž@"!ä*7?ù¶È™aev?Åʨ…DÎ?¬°Ä¿žLB?åš>o§WÈ@ùŸM㍮¿èìðùÒ¿U¿ï"8Á½z?Ü5-vÇ¿ÏöÈlàÿ¿Ø:ÀðÒ¿£-oàô³,AGNbll3FGL J1340.6+4412RX J1340.4+4410?ïÿ%`ÑjÛ?uâcE2€?Säÿ‰mp?uâcE2€?ïöÔd¾?V1®W†?RW6²–ƒ ?V1®W†?ïøxyäG"?=+3sŽÔý?N]ÖØ\?=+3sŽÔý?ï÷-&v.??^4š?Pá¥1âU??^4š?ïÿLŸŒD?:?YmÂÄ?}§ËÀJú?:?YmÂÄ?ïھоQ'?x]nO{Ù¹?r —ŽIRÞ?x]nO{Ù¹?ïúõUÆÊÄ?]¯¥Ã÷"?D*§÷ã?]¯¥Ã÷"?ïëó<3s0?W CYõ6?dÃÉÍÏ?W CYõ6AGN4FGL J1340.8-0409?àO5ó,@LA]€ä–îÀ:Tò÷ÙÀÑÀ<^=ç™@µ|I| º?þ®³Ý¾?ÂÓë9Ÿ]ÿ?˯D%ɾ%@
jOv@'g…d¿ïԖZIør?ïÿþBe«+¿Ùì ºŠªé¿áÒ°;œŽA¿å®úS¿ïúX¡+ß,AGNbll3FGL J1340.6-0408NVSS J134042-041006?ïñ½"ãø?WK]Ë\C?\"Ø£ÿª?WK]Ë\C?ï·¿¬JB¼?…زZÆû?'ð†÷?…زZÆû?ïªê+yÍÄ?"õµa;ÓB?…Eu/Jþþ?"õµa;ÓB?ï…lôӄª?rAÓ#óä
?Ž¤Â½`et?rAÓ#óä
?ïÒt'+IJ?t´•ïyÆ?vŶì-j½?t´•ïyÆ?îÕÖÛÞ'?°I)í‹Ê~?¢®â•±¹"?°I)í‹Ê~?îeM×EÃü? "Vx´?©«"ŠÇÙC? "Vx´?í§|VùÈ?Ò‹Äà?²ÄGUØc?Ò‹ÄàAGN4FGL J1341.1+7433?ä†??#€@EI¾ó(À;õÙ7>Z¯À=8XÍ@!m¡™?ý>½c£>?ξ¿ƒc!b?±í{˜ý'g?èÙ᝿C!@Wê°¢¦¿ð?ïÿùJYQ¿ß ªº©3À¿ÝmS?˜j¿é"Î^G^
?à…ª.<SmAGNbcuWN B1340.4+7450?ïþÅý0B?+Cxß-¼?#¯ãȒ܋?+Cxß-¼?ïö³V•I9?T8ð(rî?R™Rlùng?T8ð(rî?ïlÎᕺ?'8"áJk?'f<j¬€®?'8"áJk?ïùÔw-?5/"Ô²¶¾?KŒ®šö?5/"Ô²¶¾?ïþE¾ƒ¼k?-`HæT$Á?+¤VEÍc?-`HæT$Á?ïÜY9Øü?vl•VHI?qÓc#Éè?vl•VHI?ïp¶ŠQc[?'Ìs—™'¢?'é.¼²Ì'?'Ìs—™'¢?ïäpòè&?`ܝÖdX?knôZªx?`ܝÖdXAGN4FGL J1341.2+3958?èח˜•k@RaÞ¨—cÀ:´4'D¤À<ÐÚx†ú@ ›Ó¾®{ÿ?þUÃKCË1?¿£«@`¿";$wj¬?Ö¢WBÜôb@üP#ÙÎé?ïúÖ*C i¿à*·ß)ñ–¿è?¯Èe_¿¹¸þæ$¿×ú3ÂûڿގH,¿{«AGNbll3FGL J1341.0+3955SDSS J134105.10+395945.4?ïüõDBØ ?.5À@ž??8UÝY1Äì?.5À@ž??ïõ.@bÏ6?h–§>ó?U£~û(Äá?h–§>ó?ïóÈ?°€L?HPlŽ¯"?Xo³×%?HPlŽ¯"?ïìú½©w?Ggq÷]?côk'Øâ?Ggq÷]?ïùí
Mà"?C>V	?HKÊØý™á?C>V	?ïÙw¬5ò?y*èzÝ?sD)á¶úå?y*èzÝ?ïò2Çþ[æ?iª)áå?[špJÀ"?iª)áå?ﻋð[•?onõV-ß?ö¡ˆÚ?onõV-ßAGN4FGL J1341.6+5515¿‡ž·KíOŠ@N7°ËæÀ;«GhGÀ=Í 1cO@˟P<ÙO?ÿ0–‰B?Õ6]ŠÒ?ÄAꛔÆv?ðÖN™@°	j¿ïÿ3Qf$!?ïþ5$¤ú÷¿ÉŸF—> ¿ÝFéÞÖd¦¿ì.U'ÙŒ?¸Y:®Ò'AGNbll3FGL J1341.5+5517SBS 1339+554?ïö։l®]?K|{^7ìj?RRìÔ,§#?K|{^7ìj?ïñ¹ÍtE?]Ú2$&e?]ȌrÕå™?]Ú2$&e?ïwˆ
ïƑ?…¹]?‡e¡?'þJž3Ý?…¹]?‡e¡?ïÓFCä¹Ü?\¹¨€ß+?v\Þî?\¹¨€ß+?ïç¯f+ûS?bÏÞÒÞÂ?hP™Ø$5?bÏÞÒÞÂ?ïËcç8¼h?z¼6)mD?zNm@´?z¼6)mD?îþ¶'ޅ ?•ïPº•ƒ.? 'ó•?•ïPº•ƒ.?ïD˜'™í?…¢TÁ1êÝ?—lìH…XY?…¢TÁ1êÝAGN4FGL J1341.7-3907?èìr$hGÆ@6·Žâ†ruÀ;›¡Ÿ!˜×À<Á_s-F@!ë¹½ûN?øŸåÉä?ÖFlÊS?Ĝ:HPPÐ?ên±XÒÿí@AP5ÍlZ?ïâkªÛ
¿äòõÒ-_¿ïôo"͊?ï­œ®÷пë‡ùÞþ¨'?ß¾F!L€âAGNbcuPMN J1341-3906?ïø1rá?MB(/- É?O¿9ºü­î?MB(/- É?ïï7&̌O?bÖsÄdʸ?`ÈÙ3s±?bÖsÄdʸ?ñ*Ù?"k¢kGr@?‹9ãU¿?"k¢kGr@?ïütù.Þ?34¬e%­?<X8—?34¬e%­?ïílר?d*hÜ|á?b"(½>´y?d*hÜ|á?ï¾dÉАs?†v"khj?€f͗2™(?†v"khj?ï^å¾É?Ž\áaÂ-[?"#]¯?Ž\áaÂ-[?ïñ5è¢ÉÍ?Z¡¬6¤Ó?]".Lxçc?Z¡¬6¤ÓAGN4FGL J1341.8-2053¿Ùæ™&­@D:[–(ËÑÀ9ÊàÆ~ÔòÀ<†Ñ?ù@ÿ¶YÃÀµ@t"« «?¼~)¦—ƒë?½[K?Äf!?ú4§Ý);c@®ã‡¤z¿ÝF—"Ûâ¿äñiϧr ¿èÂSAp²¿êªüóF¿éØêýºU|¿ðAGNfsrq3FGL J1341.9-2053PKS B1339-206?ïþ0¶Åé?"Ç€AS?,ô•õ]¥q?"Ç€AS?ïôPiné?[œe.‹ŒC?W_-ªåž¹?[œe.‹ŒC?ïà¤åš?g@
Œ/£²?o[÷µÖ'?g@
Œ/£²?ïþ²X_ñ
?º¿˜	™?$ÚvHÂ(?º¿˜	™?ïÿ§/aö?+¦2¼?‹fgŒº?+¦2¼?ïÐpJ7S ?xtƚy·?wÇÚðµ?xtƚy·?ïɔP¯oð?}frJ¬>?{5׌Ë(S?}frJ¬>?ïúXWÑ	?;@§tð6?FŸš"%"†?;@§tð6AGN4FGL J1342.6+0944?äé']ÿÔ@Q4Z_Çæ´À:||ûÀ<€"ï5­a@¬ƒV6C@‹°'ݾ?Â77º+Šr?¶ÎùwМ?õL{ÃŽ@ª²W*´4?î°ßóE2¿Ó֑ýCD¿àéâoܿߥk*±¿ç2F8Éu)¿æ–øÕiSAGNfsrq3FGL J1342.7+0945NVSS J134240+094752?ïû©…¹¬£?d'Ó8‡•?AYêW‡Ë?d'Ó8‡•?ï킖ë
ó?g -xû¯?b}i<Ѕ?g -xû¯?ïð'Ì3!?pۀ!¸?_°gÈ°mO?pۀ!¸?ïæ&hۜÚ?NŸÀ¹Ñ8?iٗSÕB?NŸÀ¹Ñ8?ïû"po¨?9«Rp9ŸÆ?A®?ÀR|j?9«Rp9ŸÆ?ï·è³¡òG?ˆ¯pES?'ÓÛd"?ˆ¯pES?ïáðֆ?|0j
ʱ?nîç±Ô?|0j
ʱ?流|͟Ê?pcˌü?…Z Щg?pcˌüAGN4FGL J1342.7+0505?ÖÂ-ê
Ë@P3 ٔ[lÀ:…̹–nÀ<z
Á$"@´¥§nïL@lFD‡ïM?¼èÁÊæÌ¿`àéè?rï‹y×m¡?ÿÓhõâŲ¿Â´†…ß¿ßíÞҞ¿çpLÎå«Á¿ãAãÀe»¿ëp8à?á¶?Á8AGNbll4C +05.57?ïðX³}ùß?Wãý$âB??_N™*‡â¾?Wãý$âB??ïëî^£'?hƒ/ðS?d¡Ñ>&!?hƒ/ðS?ï"ÿ×nÄâ?…ûÖÁ'¹?ŠÀ
+-ÿb?…ûÖÁ'¹?ïîy¬A?O½ˆŸ"?a~†@¿ï_?O½ˆŸ"?ï"×KšŒ?ŠæE'&$ú?ŽÊ-0í?ŠæE'&$ú?䥨é?'!¸õE
"?ˆZ†à䙹?'!¸õE
"?ïXßÙt?Máªícw?"íäMo?Máªícw?oCÚ ?}Íêí;ݝ?ŠÔ$ÛL?}Íêí;ݝAGN4FGL J1343.6+5755¿ïò{½w@LïQ½aõ¾À;CP8&·ûÀ<ÃÕ×7‰Ú@½ÃIâ¢@ÊOv`?Æï8&&Z¿"-"®jƒy?½*¸TÌ`@ëÓSú~?ïÞ>y¸R¿ë³â…›µÔ¿ä™V³jû÷¿é©YàÆÿ®¿â7EçjÞ¿ïú°€²AGNfsrq3FGL J1343.6+57536C B134209.5+581020?ïÿHñœ¡?püÓÕÍ?áËÆ~¤y?püÓÕÍ?ï÷U?³°W?UE…²êH?QU€0+1Ø?UE…²êH?ïñߊƒjó?HYœÔHv?\@ëèŠ??HYœÔHv?ïû>÷Ùã-?.Š/ÖsË?C è2`?.Š/ÖsË?ïÿ¬17?I^]‡7q?óÌf¶è?I^]‡7q?ïàŽ›ÂFj?oÀ¬Êx/¤?oqd1Zþm?oÀ¬Êx/¤?ï祤‡ÿ?kA
L<?hZ\é?kA
L<?ïå…<·¸¶?\œÆŽçÁ?jzÃBÇê'?\œÆŽçÁAGN4FGL J1344.0+6605?Ž©Em¤F'@I™" äÀ:›wTË3pÀ<«"¶
+@–6ükuð@äìé¢Æi?¿8Ȑ‰¦?°£€ùÊ?íºÞEÆ@|™ÒÏp@¿á¹€¦ƒ¿â³Eqú_¿ççb\«¿æ¢ ©XS~¿â¦t©H›¿ãŸsbÎ+rAGNfsrqGC 1342+663?ïþÎbà0=?
¬'ë?#Ðϸ	?
¬'ë?ï÷&'ÿ+ø?TYѠЩS?Q²úäŸn?TYѠЩS?ïõV¾J€?d|­A@÷?URƒ`Â?…?d|­A@÷?ï÷ìäLù¶?5è/"!'?P&6öÿš&?5è/"!'?ïþWxž?%åRƒÚÍø?/z‹j–Ny?%åRƒÚÍø?ïßt±F£A?põ'Ï‹?pE§Ipr?põ'Ï‹?ïöîÍ_n?`躽Kg—?R"e炴?`躽Kg—?ïÕK'Mð¤?d8ÙUëE¾?uZ7peÿ?d8ÙUëE¾AGN4FGL J1344.1-7700¿ÕgiÖÀ,è鳍aÀ:j{Ö:3ØÀ<_ÐJ/Ï@dá59°@ðÏü,5é?ÇߋÁ>Ï?Æ˦‡ÙL?ùÂ=ý'·?õÂ/)ä*¿ïïwÀOç?ïþõU9¿æRÝ^ˆ¿í©·ôÎs–¿k*ýžj¨"¿èk¦âWxAGNbcuPMN J1343-7658?︊…!	?¡Š/ó|}Ä?Ý^¸Å ]?¡Š/ó|}Ä?ï†I 8i?—~ñQ)?Žm·ë­«?—~ñQ)?ïóÞoÈ¡?•
Q`ë‰C?Ÿa"3¾¹Þ?•
Q`ë‰C?ï¿Ö"r+þ?pµ
º¡W¥?€
wT®®®?pµ
º¡W¥?ï@|Æ8O?š&1ùêj¬?—ðg'¨'?š&1ùêj¬?ëÃÇ["ò)?ÅfòUrx?Àðâ'ì7\?ÅfòUrx?ì²Ïíàæ?¬<"2k!?¼i€øÐ?¬<"2k!?ë൮¼Û,?µAßtIqò?À})E"P?µAßtIqòAGN4FGL J1344.2-1723?ïýÞ¨v¬@EÕ¡"úÖËÀ8ðÍ¬üÀ;Õàl¼Á½@.÷"ûR@ÙªæÈ÷U?ª´vØz?¿-¯e³¹@ORáNd@ãؖÚw…?Û´;ÿµ'¿Ùs8œS³0¿ã'Í¥&Á¿áš¤'D`'¿æÄì=ÖOX¿ðAGNfsrq3FGL J1344.2-1724PMN J1344-1723?ï÷W†4ô?j+p@¹¿c?QPóØb"?j+p@¹¿c?ïïÉ'q:?dK͊ï&#?`6é€Ì–	?dK͊ï&#?ﳤq
?…|™ó¶?ƒ9VÖ­ù†?…|™ó¶?ïþÓlùþ^?8äYÈK?"É1žõÚP?8äYÈK?ïøí7․?EãtPÇ¢–?LK w£¤Ë?EãtPÇ¢–?ï¼Òfƒ†?ŽÅ}ß:ï?€þËb—Œh?ŽÅ}ß:ï?1E*?‹6ž×?‡3È}‰x?‹6ž×?ïý?D—?*ÂHe¼l?7>JTn?*ÂHe¼lAGN4FGL J1344.4-3656?í-ž/Êå@8¼%á;ÛÀ:6,PÀâ´À<G‹³ýÉ@Y/'éA@£Cœ7Ì?¸Ñæg'¬l¿tª÷ºâ?ã_v¼Ï)@:î¿»Â8¿ÚËÅ:Ý ­¿äpŸ¥LU¿ä´àFý¿å=µ¢ä›ö¿âŸÐJ/Îû¿Ô‰þ¼3!•AGNbcu3FGL J1344.5-3655PKS 1341-366?ïùwޑxì?=?("µšW?J †¶rÐs?=?("µšW?ïí©Jg?eâí"UN?bàW#îhÉ?eâí"UN?ïⲌQ)
?põÇ¡xì?mMs¼•f?põÇ¡xì?ïñ2µ^ñþ?D)L>S}µ?]š•¸N"ž?D)L>S}µ?ïçeÔ4?]j]›®s#?hš+óÍdq?]j]›®s#?﹬ïŒÀB?ƒÚ+•'?"ÄÏïl?ƒÚ+•'?ïÓTåµ|?{ю«éx5?vsUnè².?{ю«éx5?ï™c `Ș?z¿'»z³?‰§7î­	?z¿'»z³AGN4FGL J1345.5+4453?åQ ±Ü1@QM#c²WÀ7&Š
4›éÀ;q%SvŸš@|Bµ²)@^á77¥?‹›ó]|ªB?³øf>ßu@&y•în@ »ˆb¾¿À
lÐó.¿à Êƒ+¿ä²+@ "¿äk¾§›¿èÚ^Poˆ¿ìܞÁ̓—AGNfsrq3FGL J1345.6+4453B3 1343+451?ïëPNÅ`?b½—ÔL×?d¯â¸Ø?b½—ÔL×?ïà`T­4?}œÆ©Uüò?oŸâ'5Ä?}œÆ©Uüò?ïÀTŽ*@?ƒè9zÎ?Õ¹ç¿æ?ƒè9zÎ?ïô÷…"ˆ?W…7!«Q¢?VÿDàh?W…7!«Q¢?ïÕØ"°?lö8Ú¨´À?uî·¿²¦?lö8Ú¨´À?ïlâ©­ãÓ?±›¥®íí?'cªÅ˜?±›¥®íí?ïÁ:̞mƒ?"½Ô¸pÎ?b™®	Ž¯?"½Ô¸pÎ?ï»GP{¸?{µz*}~ô?.+ðÊ\?{µz*}~ôAGN4FGL J1345.6-3356?ÀºXO'&@;—BöÖÀ9ýžóu®À<PS@ôÄ@¾wÎm¶½@W]K4²?µž—°5gk?"?\6a»Ý?Ѷ»"i@+(wÃ[?ï÷À@win¿ääž_Ñ÷¯¿àýXsHͿ㣮¡£S¿Õú7¿	Ò¿áž$˜¼AGNbll3FGL J1345.9-3357NVSS J134543-335643?ïþ-ë©9}? ç>»‡…?-!Bðã¡)? ç>»‡…?ïô îD
C?[‰¥I"ã@?V¾#Vé;.?[‰¥I"ã@?ïòPS÷ÆB?iŽ4/5ck?[_Wò6ì	?iŽ4/5ck?ïÿ§A;ÎQ>õÒúH?/¦ƒ‰åQ>õÒúH?ïý©Ÿ(ØD?/~as¸È?2³ìd­?/~as¸È?ïОŸ×?{<áÄ=ú'?w°¯óë¥ ?{<áÄ=ú'?ïñDi&Ë?m'":ò}?]w-àð9ž?m'":ò}?ïÿUåS›? ¬HêÚ?Dâ±^É? ¬HêÚAGN4FGL J1345.8+0706?ßS–Æ疹@P‹6¤û©À9lì®êc·À<7T+Ñ?"@‰gWË@P†å?¯6lx¤,?ªíŽ
t]?÷@ô@g)™¬c÷¿ÐB~ª¿ãWZYé¿åÎU-XþŸ¿çí`Á
ø¿è¯>;¤ò¿áìÈ×'šAGNfsrq3FGL J1345.8+0704TXS 1343+073?ïþAYÚð?"»ôvUºü?+è@–ï?"»ôvUºü?ïó>,¥>W?cVqîÞ.D?Yƒ¦Ö'M?cVqîÞ.D?ïæ±m?n¹ðòjÇ?iN㧗W?n¹ðòjÇ?ïÿ™jõ—F>ý½¡í|'?	¥>ð"Ä>ý½¡í|'?ïýf Ñyã?/€ùä^ é?4Êùí#$ä?/€ùä^ é?ïŧöÃZ!?'ÃS²?},£ÒOg?'ÃS²?ïÔ#øÐY?zúe"ÏÑÐ?uÿp?zúe"ÏÑÐ?ïÿ8cx?@nZEeË?ó¤€j˜$?@nZEeËAGN4FGL J1346.3-6026¿ÊëÏÒ1?ûL'à°«À8q¡ueÀ:¡6¢S|@''•>@-@˜ÿ%­B?°üñ>~–?»B	å²@
ßËâ˜?þªFJ?ïÿÿ" 5•¿Û[gð$–¿ä¶0íÖ¿äù'c€¿èQ
I/û¿éÊßâ©-AGNrdg3FGL J1346.6-6027Cen B?î
jn«%Õ?µ´û·hXü?¯YY½>¤?µ´û·hXü?äŠå'Œrü?ǦB»L­ê?Öê4úç	?ǦB»L­ê?çüNGê?²ÿ‹;u—?ÑüÇcp,?²ÿ‹;u—?é5'ÙÛ˜?¥0]Ëû%,?Ë+`˜"Ÿ?¥0]Ëû%,?â¯ãVڋ?Ì+CZr½7?Ú¡ð9RJê?Ì+CZr½7?±Õù÷FUÌ?µ;d!k?íÅ@Á2²&?µ;d!k?åø†qý&?·ëæÙU€Â?Ôó³ã?·ëæÙU€Â?ÉY'ùÖ+?«wAzÕ¦i?驟AŠu ?«wAzÕ¦iMIXED4FGL J1347.1-2959¿ï̏»z@?[4ø/Q&À9ûŸÓo~=À<BÙÊQm@æÀ3â/µ?ý"ZÖk®?ºbg÷¶?»à€&(@t G2Ä?þØépq'?散ª?Y?Üg¬Óª7¿ÜxÏ>ìúÀ¿ØÍËz¿åºçÇúÖ¿×`óà·æ6AGNbll3FGL J1346.9-2958NVSS J134706-295840?ïùÚ±‰FÞ?=ª³yìäp?H•9˜ì
V?=ª³yìäp?ïu¾¿Ý"à?"Èú2Ë)@?'H(¼ÿÿ?"Èú2Ë)@?ïä$®F`?mÎü2nÔ?kÛQóYRÓ?mÎü2nÔ?îå|‹ì²Æ?'f#Üç>Ä?¡¨7D¤o˜?'f#Üç>Ä?ïæ!׍'r?bÜG¯è?iÞ(cOFk?bÜG¯è?î/¥SÙh^?µT	èàI?­ª¿ÕÅ#?µT	èàI?ï³çª0?…d"8¥G?ƒx;ÿ?…d"8¥G?ë³¢ëc!?§SKÓÿKC?Á1tRs|?§SKÓÿKCAGN4FGL J1347.4+7309¿Ùˆä•–TÁ@E¯BöÖÀ:øˆҜÀ<ʔøJ)@‰ðP4¡@)}Ý{pº?Å·?ªô²S.?âÍ,n@/†—3bÙ?ï)Œ‹"Y¿å|'€Æcý¿ëϒ_µ¿á¥Ù]ÔÇm¿ïÿü¿ÙŸC?Þ{©Y*=ÁAGNbcuNVSS J134734+731812?ïünKÉ=\?@üq$Ó?< zR?@üq$Ó?ïöئ—%m?T
ü<…þ?RN³Mgv?T
ü<…þ?ïÕø|uhÚ?wKiå3¬?uÁ¦_?wKiå3¬?ï÷Gˆîá?<·=ƒ|´?QpîˆëíÁ?<·=ƒ|´?ïüÁȯ?Ht^÷‡5"??èô×H?Ht^÷‡5"?ï×݅'â¬?v7áÕà?t=@Ý}»?v7áÕà?ïغ³3e?{2}kŇ?s¢¦]JQ"?{2}kŇ?ïÂú¦yÑÓ?p ÀŒp
÷?~'¬¯ÙF?p ÀŒp
÷AGN4FGL J1347.6-3751?äôdjÛ£@7¯ŽŸj"óÀ:‡©­
À<ô¬å§@æ#·ë_@[r>á½?º™+"î?É)I¥e·@
£ @¿ä@™!ç±T¡¿€¿^Ð	A?Þë®9cÎÜ¿äßâSFÏ¿äÓsëUN¿êqZ€a¿ïÿl&™Ç½AGNfsrq3FGL J1347.6-3754PMN J1347-3750?+7
?Œ©¸w_šá?‡žõ+Ä1¦?Œ©¸w_šá?ïæ"dÀN?uÐÔ­q^?iݛZº3?uÐÔ­q^?ïy›.f'(?†ÿúbÌ?Ìš:ó?†ÿúbÌ?ïíqßÊ?EYéÄp8?b~êfD¾Z?EYéÄp8?ï54ó°?LB0£¢?žýù^ˆóð?LB0£¢?ÿ¨'?•¸{¡	?S€†€½?•¸{¡	?ëõ%'ú?°0èòމ'?Ê+k`?°0èòމ'?ï­¿&­$!?p¼D»…?"6Jh#Ã?p¼D»…AGN4FGL J1348.9+0756¿½GÊ)@Pì¿±[WÀ;'/Lô¥YÀ<ŸÀ_@˜@ 6Í.Çhµ@cpÍÈuO?Äái§c†¸?{ó¦‰?¸Å›€#¦Î@°Î‰»U+?ï!
÷9ˆ¿äi;,ü¸M¿Ü4…ãÚ/Œ¿êq¦ é4¿¼am¿\]	¿Á§Â盰AGNbll1RXS J134853.8+075704?ïýâï×qt?0@³VM?0èP-B?0@³VM?ïðšg¨cj?dɁ¤6T?^Ë0ãs<™?dɁ¤6T?ï陽A?p2Ñ·`à†?ffý
e]J?p2Ñ·`à†?ïýùKõª?éÜ2›?05žbþz?éÜ2›?ïýµØ",?0Ÿ®~c/þ?2Q9À¾ü°?0Ÿ®~c/þ?ï¿Ëm¸Pz?…r8Cͼ	?€
$†í!…?…r8Cͼ	?ïðjPè?nô‹~‹Ä?_+ãCíÑ»?nô‹~‹Ä?ïö¢ÆéÞÖ?Ià·¸+¸?Rºqí	ƒŽ?Ià·¸+¸AGN4FGL J1349.5-7153?íUžìPÀ#¾è»¶À:^qS)rÀÀ;æ"4­†¶@:û³•V@Çc»';?»œ
7;€Š¿³ivRˆŽ?û
6 ¥ý?é8.¿å˚gõ²Ÿ¿áu³Á
&¿ìã4–~\¿×çâT1¿á½'á>sÙ¿ÖFÁ#>AGNbcu3FGL J1348.5-71502MASS J13490974-7152510?ïõ!³6¬B?W8ÌݎE?U¼™tìm?W8ÌݎE?íø_àîËX?³jº‰±?°=úAs??³jº‰±?>%C?‡|Â)wöñ?‰Ø<3æK?‡|Â)wöñ?ïƒ"û
U?xÕBR¹?;7H¢™?xÕBR¹?ï«ÑM¡.Ê?ˆXwgð?…¬"D±e?ˆXwgð?Ýù7—yŒg?ÒB|7ð?ád4C9Í?ÒB|7ð?îàÓ¨;Ñp?™v5Ô\¿ó?¡òÅy¯4?™v5Ô\¿ó?æԐvÁd?À=~"õ3ã?ÓÈVß}9?À=~"õ3ãMIXED4FGL J1349.5-1131¿Ñóxˆ'u@HnR'ƒÓ_À9Ñ×ΈÀ<Ñqw;¡@gŽiâF@køüÖÔ?±`'?º×ù%Æ83@1ù⯍!@¿¨ƒÂAÙ¿Ùò½'È¿âYLV¿æ¡*òòÑC¿èò™°?ÎL¿éÓÔޔ‡¿ðAGNfsrq3FGL J1349.6-1133PKS 1346-112?ïýŠU¨³?*Þ\¢a›?3­Uñ…AÆ?*Þ\¢a›?ïõhŒäÞ?\\dûf?Uï.Çù´N?\\dûf?ïâ¶)áë?c|0ÿY˜t?míI±M®?c|0ÿY˜t?ïÿ¶"¯­‹>ù8Æø_Ü?ZáÉ`@¦>ù8Æø_Ü?ïüÔTýç?3#Þ¾X÷?9_>Æܸ?3#Þ¾X÷?ïÍÏÍ÷Þã?Içd†œý?ypft?Içd†œý?カn'?z2rWY-?€'\žôoÒ?z2rWY-?ïÿƒä",(?úDqzÿê?Ø#?úDqzÿêAGN4FGL J1350.8+3033?â}íRö"i@S#'©"áÀ9¡%t9ŽÀ<xáR•Ï@F•[œ]ï@ÚöƛZd?°%ºç?·'.~SÔ$@f¡aä÷f@"·wP?ÒXÖ%;"ì¿âRñ©ûçm¿ç8⟜é¿äc²¢)5.¿é'ï~R–P¿ïÿÅbu@AGNfsrq3FGL J1350.8+3035B2 1348+30B?ïü!–3?31ŸY8h?>óM¿Ù*¥?31ŸY8h?ïöÂ[§ ?Zë|èïOQ?R{HØW`·?Zë|èïOQ?ïâ+½·ÊÌ?`F?'ál"?mÔB<´?`F?'ál"?ïý{šÈ»?#ɑƒ°Í?4'D,Æ?#ɑƒ°Í?ïø†ÈöBV?E-ȟh¡?MäÛPM?E-ȟh¡?ïØqdàï?'²øhÔ?sÇM±4¨?'²øhÔ?ï¾óyù…?ˊ%´ú±?€xCBŽË?ˊ%´ú±?ïûSæ\ÿ?4AlåðâÄ?B°gcà°§?4AlåðâÄAGN4FGL J1351.0+0029?ê]ê–â/@Má;:h±šÀ:d­
ê¤NÀ<jm÷È@¡lÅûø4@âmæÎ?ùY}tË?¹•þÀ¡§?õ%b?8È@vÙÑ4¿Ÿf…Åý$Ù¿ä	•ao1¿æšÔ,<ží¿à¨1ý©
«¿ïþpHgwÞ¿êrÀü§†AGNfsrq3FGL J1351.1+0030PKS 1348+007?ïýx]"´¥?(M£øÉO?4=#‡®?(M£øÉO?ïó;uï<Ü?_ÍÔ@×ß?Y‰ÁQ9F?_ÍÔ@×ß?ïëAúÌ9?^:qà&ú ?d¾É"?^:qà&ú ?ïþ˜ÍI|ÿ?#$æyþ]?&s)7oϏ?#$æyþ]?ïþžSg±? !/¡G['?&ÉI£? !/¡G['?ïÈùôMDV?',µë‰ÑP?{ƒíK¬?',µë‰ÑP?ïîTé*?]?l·:*$—?a«{RB?l·:*$—?ïüwËyÍ?1Dç̾›B??A @›0?1Dç̾›BAGN4FGL J1351.3+1115¿Ïs†žj@Q1›€#¦ÎÀ9t™kvp À<
cu^P@…oòbü?ý+þ‹‹º?±@¥\ˆ?°¿ð©Jè@¯\äÝdË@á´¼µ¨n?í°çɨU?¹ðQJöH¿Ü"÷ž\¡ì¿ß"S¼ëƒF¿Ôk•D C¿äM~8C"AGNbll3FGL J1351.4+1115RX J1351.3+1115?ïþ/á5?(o¹h½Œ?-ð‡rh¾?(o¹h½Œ?ïëe 7¥U?m™º‡Ty?dšß×xòº?m™º‡Ty?ïîKSª:ë?kU/Q
N?a´¬ŒE?kU/Q
N?ïçêã
Uÿ?R'ǹ"?hÿ™
?R'ǹ"?ïýý>…?2Á\œÓý?7_˜Íª-4?2Á\œÓý?ï¤$Þq;?™Ë
LG@?†öȍ'½F?™Ë
LG@?ïç¼:§5?tòc¶¢?hCÿžÝ+?tòc¶¢?ﻅÍ3úÙ?ry;"q'ß?Œ¼ 1Ÿ?ry;"q'ßAGN4FGL J1351.4-1529¿ïÿë€}@F|SŸºEÀ:}«fJ·´À<`š¡×U½@­ïõEçÁ@ÃÙß?Á»»?™½)Íó?Û¦£Æ™,@""ì¿ÞB#ßX@¿Èš×‡:òD¿ä1YtœU¿Ù"öd ¾|¿ã\YýL¿Üß齃AGNbll2MASX J13511746-1530155?ïþ›º8Ô?.Àù±YO?&DX¢a?1?.Àù±YO?ïóþwiÃé?ZŠàƒ4ë¬?X¢ª½k?ZŠàƒ4ë¬?ïøÝ®¾¼5?9[Ù:Ö¥=?L‰DÁý1¦?9[Ù:Ö¥=?ïüƒ€?#ªçò<?;ãý÷*Y?#ªçò<?ïþ*@¬~µ?#'éÍ¿^ ?-[øóâa?#'éÍ¿^ ?ïÆUçéì?€c˜…çBì?|Õñ_6?€c˜…çBì?ïû•Ë!?P¼µžÏ
Ú?A½©1±—‰?P¼µžÏ
Ú?ïôJò…??FOka¼ï?Wjrb?FOka¼ïAGN4FGL J1351.7-2912¿Úڒß&|Ó@?օ3±tÀ:J4ÿ¼
bÀ<.43
s†@³Ç­ËÖ@=•!dԖ?Äab*Âv?Ð0š<+ÕF@	¾È'L@K8P©f?å}d¸|߿߀-·É/‰¿å+¦—㷿噹Å¿ïÿúVrÓ\?ïÿÄ`"AGNbcu3FGL J1351.7-2913PKS 1348-289?ï­Ô.ôgÏ?‡¥—kÑf?"Šô5'œU?‡¥—kÑf?ïï T'Û=?cµ›ϕF?`ß«…'?cµ›ϕF?ï€ü®€ ?".ô…§®?Ÿàq#ï?".ô…§®?ïõ"¡ü¦?DÖq°êÓ4?UͺwN"â?DÖq°êÓ4?ï5ñ˜J?š¬_fdZj?™LAƾÊ?š¬_fdZj?ï­Ð¾|…•?‰Ãj²Ø-I?"‹Ð`ޚ³?‰Ãj²Ø-I?ì†Í°Ö'?§±(Ë^	?»É"zyKy?§±(Ë^	?ï™]åõxú?~ìö×?‰¨†'¡Á—?~ìö×AGN4FGL J1351.7+5542?éÐärø@M´¥œ[dÀ;•Ùs¤<‹À=<ÖJ$@ŽššuŒŸ?úŒõ–ðqî?ÒÅ%îÇÉ?ã‡/iz@".C	j@´Äî1!¿Ïì\	@E•¿ïZu%F?ì_Î1PÚä¿×álˆ€Ã¿æSÿ¨Â,¿ïÿøþÙå9AGNbll87GB 135011.8+555656?ïúüꐛÞ?NÜÆJ:]?DV­^"?NÜÆJ:]?ïáMq*˜?wk`Qè?n㲗w½?wk`Qè?ï¿{oPà?•dO–ÞVÍ?Ÿ^?•dO–ÞVÍ?ïh룞øv?yëi=ƒàŸ?'â‹'H[F?yëi=ƒàŸ?ïõwx~ä?a	'̸)N?UÙ¬
x-?a	'̸)N?ï­´eš0?•ª|‹ƒæ±?"'æ S4??•ª|‹ƒæ±?îò¢àÑLÊ?™º€hýt? ÕÑóÇX?™º€hýt?î›Î ‹?"ŸÊj"É¢?¦CÒîT?"ŸÊj"É¢AGN4FGL J1351.9+2847?íKˆd=a@S"T6¸ù±À;' ŒÒáºÀ<î%ÎÆ¢@Š·ÖpŠ?üýŸ‡Ü?ÕËÛø8á?Ìmñ	Â÷a?ø¢³ôŽ²¶?ÿ¿iÒ~¿ï¤«{Cm=?ïëu™àv¿àkTñ¿Ðü¸''ì׿åévP¿5¿ïÿ'R}{AGNbllFIRST J135154.4+285007?ïí¿¦ý
?^¢rû%Í?b@Y8ŒØ¦?^¢rû%Í?ï²EםÐ?›ÎG€…?ƒnŠæõâ?›ÎG€…?ï­ÿ"ã;?E¹'DP?"€ùrˎ?E¹'DP?ï†]S\_?rQ´9˜Q?Žh«%L<?rQ´9˜Q?ïáRÜ#Š|?k–®¨Øzx?n­#îS{™?k–®¨Øzx?ï
+£¶—Æ?­3ŠÌP?žZ‹Œœ£=?­3ŠÌP?ï7èi‹^î?'¨SÈ^f?™òΔ"6?'¨SÈ^f?íÇøÍMÉ? "mµ~ì?±À?8K·>? "mµ~ìAGN4FGL J1352.7-2742?ӄsá½äk@@œ°À&ÌÀ9ïHk©œFÀ;鼌ã©@‹¥ÝIǟ@M_Âví?ÁlÙ݁zê?ÅPžéd³@é¾àzÿ{@]¤í_¿X¿Õ8~âHN¿èJ€Â2?¿è.ewS¿ë@˜Á­^ó¿ìKt½Âè¿Ù¿†ÞV&AGNbcuPMN J1352-2745?ïîåÄü…?†àÐ×÷·Ø?a;xxj?†àÐ×÷·Ø?ïî¢o"š?câÓÓ0þø?a]'¡O‰?câÓÓ0þø?ïÏló&?qÏÈ졶?xI†‡Ê3r?qÏÈ졶?ïð˜@²M?EÒ'g;1?^ÎýšFR?EÒ'g;1?ïíŒný}‰?b>Ç#6Í?bsâæ¦?b>Ç#6Í?ï°ð»ix?†õŸ¢ôÁ?ƒÃÑ+![
?†õŸ¢ôÁ?ï·ñžh?"r±Ì‹÷T?œiÌ2ô?"r±Ì‹÷T?ïdˆrLE?'èM†—3?"nñ¶w\?'èM†—3AGN4FGL J1353.0-4413?îá™9;NÏ@1D^=¢ø¾À9u –
À<ùée‰È@9€H9Ö@cZþSW–?²¹'©gB?°c¥kßÍ?ü6~â^.Š@õ¾]ž@È¿ä«KÞ$ãå¿Öì@Ûgo¿ãýMž"[¿âgT"*d¿äÌ~É3»¿ëZ0Íþ%4AGNbll3FGL J1353.1-4414PKS 1349-439?ïý]òµ¥Ð?'{£»me?5i;Û?'{£»me?ïß$pÖ4ˆ?z®QJ—?pmǒÕ÷ð?z®QJ—?ïñ·Ä89é?cAÉÉl+?\wøL—?cAÉÉl+?ï夡#j'?RŠ7ÿÞ5˜?j[^šœþC?RŠ7ÿÞ5˜?ïø­9Œ­?CAša¼?MK®‰7TÇ?CAša¼?ïGA¦:Í?¤å8F¡Ë?—Ë5¹nx?¤å8F¡Ë?ïØÙF>?€Ç œtî©?s"\ööuù?€Ç œtî©?ï‰V¶°Î?}'úb[²?ªœ¢ o?}'úb[²AGN4FGL J1353.2+3740?ìZ»ëS¸@RPñýÞ½À:øªÇ¿FÒÀ<ºjÖ7¯š@(YØ8À?þšþSW•é?ÑK,¹œn`?Å<EÖxó?ót1ËT&É@W9°$ö?ïù¿`}™¿ê:'¦.(¿á hUSïk¿ÒgC±Ý¿á¾Ÿ­¯Ñ¿ïÿå=†ô&AGNbllRGB J1353+376?ïüsÂß'?5É£{è/?<aèÔ3ô•?5É£{è/?ïôË??AE?YOznŽ?Vi/×?YOznŽ?ïä]àZô?oëПr}?k¢ÑèY?oëПr}?ïàûá?ÿ?PPï:n¾Š?oþ;œ¸Ü?PPï:n¾Š?ïûB=è??êv'¨?B÷	TÐä'??êv'¨?ïՑ©$÷?yóž¸/cr?u7+iÕüŠ?yóž¸/cr?ïÄ<¥Kù?ƒ&Xì+º?}᭄ˆ"?ƒ&Xì+º?ïšØh·N‹?uTÑ[ÜX‰?‰IåßêÍ?uTÑ[ÜX‰AGN4FGL J1353.3+1434¿ïÿ©\ÉôD@Q¸«`kz¢À9æÔø³À<e¹@þÍÑ@ !‡å<@üæb I?²˜8_[Éï?TrÈkáqí?¥(æ~#ÇZ@
»Õ§ç»?ïüü_·u£¿ä}üàeÛÒ¿ä,u©ÐH'¿â0›©>R¿äa߃ˆ¶¿éfj˜$N"AGNbll3FGL J1353.2+1435OP 186?ïþÏ,3ËÆ?&ž¿ËH?#
:¼Ku~?&ž¿ËH?ïòț©ƒ
?d!ݸõ?ZnÈÿpŠ˜?d!ݸõ?ïðԘÀx"?eOmA(U?^VΛœW?eOmA(U?ïýŽ"¬Ï?#_ÿ;2t?3‹dfd,þ?#_ÿ;2t?ïþž><ý?$ê!3²Ë?&~ëDÙÖ?$ê!3²Ë?ïĺt…ô?ˆÀAóAô?}¢Å½èò?ˆÀAóAô?ïê²÷l;E?rP	ûÿÜÄ?eM^*Ó?rP	ûÿÜÄ?ïû»½…Üù?3$uOŸ¼?Aö߅?3$uOŸ¼AGN4FGL J1353.4+5600?æìï'HKý@M…çÀn¹À;A£[º:úÀ<ºŠ´úH0@ä4µê2@‡"ƒ¸†Å?ÃÙ¹"ÆxË¿"šmÚÎî?Ñɋ¤¹]Y@3=gµj¿ïî5'˜Ì?ïíÜ|m8è¿çl]Á|6²¿äXb—¤Í¿àƁŠY5¿Áè›_lw"AGNbllRX J1353.4+5601?ïýþ¼š5Ý?B!Å_´?0
hÆð~?B!Å_´?ïöXix"'?T´ù»P>?SO-t‹Lå?T´ù»P>?ï¢z?e8'"éŽ~?`yè9¿Þ5?e8'"éŽ~?ï÷¹jÍÜË?7aäñ}ù?P*Ø?7aäñ}ù?ïüÂ_zRÆ?2u¦¾ÑҒ?9í7i?2u¦¾ÑҒ?ïÙ»·j~¾?t€ÜÉ?s"$Jµ$?t€ÜÉ?ïéo_´E—?rá¾û¹F?f 1`À?rá¾û¹F?ïÐó±yEw?ku47ÿ›?w†'$pÈv?ku47ÿ›AGN4FGL J1353.6-6640?ÙdY›Ò¯À)×⪄£À9þ…¬|ËÀ;ϏÁàá@ ÅÏþ¨0?þÚvÙ{0ù?¬ï܂ˆ—$?_¤ßʚ1?µEÀÂ}i@Èm`€žK?ïÿwD;Ï¿Ú×.(\¿â³y…'¿à?€³ï†5¿×ȱil«¿Ø"<z¯ž"AGNbll3FGL J1353.5-66401RXS J135341.1-664002?ïü¹1¥?2ï ~M:??'6'œ"?2ï ~M:?ïê-¦‰õ•?u!9täƒ?eÒY®df?u!9täƒ?ï؀P-¦?y·%æ*2?s¿×֟@?y·%æ*2?ïëKÎ	¸»?U&Có;¹?d´1ÄÌäÒ?U&Có;¹?ïõEz™µ?PR"z¾ä?UótäPõ'?PR"z¾ä?ïxm¡2!?©5gƒÙ?òKԘ1à?©5gƒÙ?ï®=ÓÓ¯É?‰Z½ʒ?"p‹BÅ?‰Z½ʒ?ïÍrrúœ?nì6ǬÅM?yFÆß2<?nì6ǬÅMAGN4FGL J1353.7-3936¿±/I c¤@5±¶€Z-sÀ;Ȃ—õT«À<ØøγVÚ@"´à®ø{?öĺ|h?Ú&Á HàD?Ú{¤üۈ?úµÄ}î@ø‰*
Àx?£!¼'õ
¿ïü˜!I{Ê?ïþ±¶ÆÑ
¿£×*©»¿Ñ³œ¾ß¤¿Ú€~ÀzYAGNbcuNVSS J135345-393711?ïûÝÝL?:šÌΓ	?C"Š±MɈ?:šÌΓ	?ïêT›ýeá?p2¬ožF?e«dxI?p2¬ožF?ïÓÝ8ïy?h¡ž…BÕ?vc"ñä‡?h¡ž…BÕ?ïõÞÁ–ã²?E=ŽWÛ3Ï?TB}:¬»î?E=ŽWÛ3Ï?ïûÆ«±Ê?>Æܚ¸?@æ*`&Š?>Æܚ¸?ï 9o"?Ñ©‡K®í?‡ñºà»?Ñ©‡K®í?ïéT	?q^(f:ñg?f«÷	JMI?q^(f:ñg?ïçÒt‡)?aéfÊ*Â?h-‹"~º?aéfÊ*ÂAGN4FGL J1354.2+6934¿Ö]s±†(@GJ»˜Çâ'À;9‹n]«­À<⟍Ï`ü@ëëêÊ8É@Ñ·Xâ?ÕlEãäìS?Ó`;^ÐÅÖ?ù|ÙÚÒI?ý€ÌC:?ïû:~+)$¿ç]=B€®¿á¾-,ˆõ¿çiÆ×p•¿ïÓ9ÎWçH¿ï*èáÖIAGNbcu87GB 135252.8+694626?ïÈâ½­}°?sßd‰˜/?{Ž¡C¨C?sßd‰˜/?ï—ikÜûw?"ìC=Ç?Š%¤þrNa?"ìC=Ç?îö™9woù?
ë&ßOÍ? –lidçn?
ë&ßOÍ?îŒc?Ÿæý´ý÷?®_÷?õµæ?Ÿæý´ý÷?ï©e/'Ø?)A<jOc?…¦¹7¥¥ð?)A<jOc?íræÑÓZ?º
Ÿ-ŠÛC?´hÉqge.?º
Ÿ-ŠÛC?í´Q‰ñ—? ÒQzY?²]s°á:Á? ÒQzY?ç¯È±™?¯Ý'w(ƒì?СâoîœÎ?¯Ý'w(ƒìAGN4FGL J1354.3-0206?ï`´åi@L‡çB™Ø"À:bÑÜFwÀ<+Z§ƒ@;ç¿ÂMB@\àž:é
?Ғ	†gä?á%'`À48@×WŸúë@¤R˜(U?àÒt¬zFî¿ák™v^+/¿é•1 6ç¿ï¬ÖøŸ¹n?ÚUÛ>T¤r¿îû¶úÓpUAGNfsrqPKS 1351-018?ïŸóȺ•?²±{Äü±²?ˆ
ØY®?²±{Äü±²?ïr,e?¯Y
¨è|?Ÿïß8™«a?¯Y
¨è|?î6¬ç?›'z:¦˜?¬žÕ.l?›'z:¦˜?ïî͇Õm?Vù¨è?a2x_!¢Œ?Vù¨è?îûÀ¿n?£ŸÍà$Õ? Cö$	¸?£ŸÍà$Õ?çvìü=3?Òo.÷dP?Ñ&х™?Òo.÷dP?é–bbJÍÚ?±oû!¦?ɦvvÔȚ?±oû!¦?î¯Hë+\¥?¢¯àÑ
9ª?¥qQ•¸¨?¢¯àÑ
9ªAGN4FGL J1354.4+3707¿—í<¬ú7@RWRÁmóùÀ:‡à	Às"À<"Ûá<ÆZ@ãZÅô@"?ÿ¾•·ŒÉ§?¿˜kàè|p?£\Ðeˆšï?ås|>ió@¦IÐÙvÔ¿ÔWQ?ãšÅ?ì¤'D`'¿âƒ''g›ñ¿áÞSÝͦ¿ÜÂ÷¡aº¿à蒀u±2AGNbll3FGL J1354.5+3705NVSS J135426+370654?ïøç¶ω?C™¾a®¾?La("POu?C™¾a®¾?ïî"å?n˜t>5?ahTë{L?n˜t>5?ïíOmjUx?`J
­ü×?b°'Ç$ç ?`J
­ü×?﬐3ê=K?j 'Wã7?"Ûóp­<?j 'Wã7?ïæH\Bԙ?cÙDG_<Š?i·£}ò–Ú?cÙDG_<Š?ï¾µùâ&?Œ:Qƒ;š?€RŸŠvrl?Œ:Qƒ;š?ïæ!7S0?tšÔMX#?iÞÉgp?tšÔMX#?î²&d)™?'Ùø[%?¤Ý™À[l?'Ùø[%AGN4FGL J1354.7+0623¿é©ù@ѵ@PøôsÀ;EÖÌ*žÀ<¬Kä ÷@ 1´XÛ?þÐßìdAÉ?×¼.Ääv?¿L'Jò—?ì°ç~~á@†,ÞZi?뛽˨	Ÿ¿ä	"ˆÁB¿à™"º\‡À¿ÐÈøÂI?¿åøžï!‹¿ïÿø]Ê5™AGNbllNVSS J135444+062249?ïþ+";º?$ °]ãå:?-H¶FÞ??$ °]ãå:?ïîrhʑ+?f•-xÜÿ+?a–úU¥?f•-xÜÿ+?ïï6Y?gÐzVµOÍ?`áðÿU(?gÐzVµOÍ?ïòö9\ÿ??'Ž¿[ý?ZÅÄ?Á~??'Ž¿[ý?ïþ…¢It?$Ècú4Ȕ?'¥Úé38ï?$Ècú4Ȕ?ï¯Ýᥪ}?—J"ÿâ5?"‡§kvÁ?—J"ÿâ5?ïð0.'0?lnÑ6«q?_Ñ ­ý?lnÑ6«q?ïе¸ð2>?cƒ"ŽƯ?w¥#~Gù%?cƒ"ŽƯAGN4FGL J1354.8-1041?ìÁë²Áó@H•žbV6mÀ9y˜éåÀ;ÿä[^Ëg@n¥ÇzS@*¬azŠ?³Æÿ> 4ú?ǚ}DNc@#»@³Nw@›°´é+R?ºªÅ»ám¿âÈ}}`Þ¿äù— ¢‰¿é[ibš)¿æ1]À¥w¿ç± @Ò®
AGNfsrq3FGL J1355.0-1044PKS 1352-104?ïòšòèì?VÚíb ´m?ZÊ,w?VÚíb ´m?ï푧Ì|	?xYå+òe?bnX3ƒ÷,?xYå+òe?ﹿý?z]xÞ,?™ÓJ?z]xÞ,?ïüóË`³k?%2þOæ?8a£§_î?%2þOæ?ïï	õU?bºIVO?`öàÏ«š?bºIVO?ï¶~À‹‡?³Qàú*?'`Oé|ÑÒ?³Qàú*?îÅeS'*¢?šNof
?£©ªËՇÛ?šNof
?ïñÜj"`‰?M]Qo‰,›?\G+&6-?M]Qo‰,›AGN4FGL J1356.2-1726¿êV³œ`Y˜@E]ȟ@¢‡À;ùÿ4þåÀ=2Pµ$:@ @ԋ2"½?øóy	YÂ?×[	T<˜?íGâb
a-@
VŸ¸g?ýø8RÌ+¿ëÿÝe¡D‰¿ØàEš¾Ý¡¿Â¢HڏX¿°¹€AS²¿êêË»TÕD¿ðAGNagnPKS B1353-171?í	…jÁž?´9_`k?·³ÔªÓ?´9_`k?ìC'f^°?»·ÓZIfj?½ãt̓?»·ÓZIfj?ìó, ¥…?¤æ¢¿e¹¡?¸fšø®ì?¤æ¢¿e¹¡?ìå>ç$? kÃW	$?¿(ÖÆß3? kÃW	$?å=+"$Üü?ȋßBk?Յ¨×¶F	?ȋßBk?âÝåÛAÒ?Ñ°¹+e•?ÚD4äI|\?Ñ°¹+e•?㥅™˜©?À_`
µCL?Ø´ôÌέÖ?À_`
µCL?áåOäހB?»ø—]æK?Ü5`6Bÿ{?»ø—]æKAGN4FGL J1357.1+1921¿îÒ[Í0Iõ@RBä¸{ÜðÀ:?
€Œ'ZÀ<^gpQ¢@‹íi>]@ý‹{ɤú?¼¸•!(³l?Ž3Š4æ€l?Ç⧋P@
6҇v×M¿ãv֋'oڿ䜝Öj/¿ë SÇþ0ó¿åèe¯‡A¨¿ð?ðAGNfsrq4C +19.44?ïÝΓ\¤Ø?¦¥qsa?q¶0±TH?¦¥qsa?ïöåÊßs?\i!µ'§?R5à\'ª?\i!µ'§?ïƒÔêcÇ·?ŒÐõÉ?
ÅmíJD?ŒÐõÉ?ïüæ¯eÍ~?+AK‡Z¥}?8ʃY‹žK?+AK‡Z¥}?ïøe°š"g?RÁ¾Ÿ!…?Ni<çŠeç?RÁ¾Ÿ!…?ï½î!o3?.Ne÷RH?€"~ÿ3W=?.Ne÷RH?ï¦Úp"r?ˆdXNˆ"³?†IdåoJ?ˆdXNˆ"³?ïíšïýJæ?Xêb;?beÈûª?Xêb;AGN4FGL J1357.5+0127¿ÓŸ2ü'ÉW@Méä¼­šØÀ:/½¦îíÀ<V8‰´IH@Ú;ƒd@ü wnÌ?Àx^ õ-"?Ã%›Åî·@oPóÇ
?ÿî>¯h7ø¿ëïþ€#&?ï	þ¡[.û¿ãOˆžŸ'Ø¿ä‰]aZ
¿âàsr¾c}¿ïÿªÅÝðAGNbll3FGL J1357.5+0125RX J1357.6+0128?ïôʇ£"?R`|œ§£Å?VjðVÇ9s?R`|œ§£Å?ï*Šb(¿? Lhë$Fs?š®®XâR? Lhë$Fs?ïÈíßct¼?sÔØâ•C?{‰\ü?sÔØâ•C?îþR'ü²?‡U 0çk? ×Ð>¤ß?‡U 0çk?ïu渘"?¦»¡¯u?'C)'v?¦»¡¯u?ë¨}˜Ôo?ÄøѺ"³M?Á_Â	œ®C?ÄøѺ"³M?îwdë"_? [Œµ÷C?¨é°qó? [Œµ÷C?éfIù¦Ó?´é¥#'5µ?ÊfØd³'?´é¥#'5µAGN4FGL J1358.1+7642?ÉLÅ!ÿüq@CãŒCoÁYÀ:ítãìÀ<¯¾5ZTà@ŠÍ©ìx@¤%t:?´,Ù&ø?¦ÒU¢ÉÄ?ðjâF±•9@wûmŸÙ?å_¢!¨q¿ß›j$ÎA¿äýýâŽl¿ãÙwÕúrø¿êþMxX×2¿ïÿŒýÿʦAGNfsrq3FGL J1357.6+7643S5 1357+76?ïü‹ ÿáÄ?.àBV¸ºv?;¢ù£ÛӔ?.àBV¸ºv?ï÷Ÿ
ÌÇC?T­[]ý?PÁãýýY¥?T­[]ý?ïÛÊâÍü3?uⶠ'ë€?rŽ‰ãž–?uⶠ'ë€?ïût+1BS?1â¾;Ï‹?B/S¹¾Š?1â¾;Ï‹?ïúkjÿt·?:«ÇöÑÖ?FRSÆÍ}2?:«ÇöÑÖ?ïÞÿaÊuZ?s*îSwÑ¿?p€O%'#?s*îSwÑ¿?ïÍF§%À¦?}ÔuUG%H?y\¬S¥?}ÔuUG%H?ïø­Þ˜•??Õ>ª¬f?MHˆ±å6??Õ>ª¬fAGN4FGL J1358.9-0703¿àò$±Kx@J
At>–>À;Ž²‹Øæ·À=þæ$Œ§@&þTb`?ù(
Jk^?×ÉÔ_hEd?çN—rwì¡@Æþ÷ÂCÝ@mI%7òá?ï­àx{;á¿èÈ¿AHõ'¿Æj!´Û"¿Ä³w¼$3¿íQÖ¤¿ì‰pÃõ8AGNbcuNVSS J135850-070403?ïžQh
Á›?"`ÍÞ
Zú?ˆk¦Þm>?"`ÍÞ
Zú?ïbóÚz+â?Gs`Âp?"¡"²rQ®?Gs`Âp?î|z$M+?•ô¡	÷æÜ?¨>¸`NâK?•ô¡	÷æÜ?îáäîÎ÷—?…XZ`Óè;?¡á±X¸–?…XZ`Óè;?îãûÉÿ,?¡›Å…0æ?¡ÎÐ@ÌXF?¡›Å…0æ?íAiõs?¾ênüÀŽ?³}ô·mf?¾ênüÀŽ?ëi³®t?°k®ÒJl?ÂY½3…F.?°k®ÒJl?ìJWì>ñÇ?¨…¹Ìk³??½­@žqÇ?¨…¹Ìk³?AGN4FGL J1359.1+5544¿æätÜÿR@Mq%F
¦LÀ9¢x>Õþ¥À<Q¸ÕŸf@v$4Õk@ã¼ûžqp?­7¿^û
'?¼û•0©@@c¦@q	@Å?à?Æ?¿Ô÷íwg?ª¿ã=]º¿ä<Ž@ @¿è«þ +ï¿ì ©¡Nš¿ßáŒAÂB/AGNfsrq3FGL J1359.0+554487GB 135720.6+555936?ïû™‡Ñ#?9#'·~m?A›Ðå~l?9#'·~m?ïótu}?_Ud¤5?Y'5ê?_Ud¤5?ï°ª!©V?"è²E1ïY?ƒÕw®ö¦?"è²E1ïY?ïä'8Ë?Rf,å­Ä?kmÇq?Rf,å­Ä?ï÷ºÈØe?I#¨Šä‹É?PŠn&¥æl?I#¨Šä‹É?ï҈,×ü?w9U£€ç?v»éŠ#®&?w9U£€ç?ï$}Z@5?–Äó©ISË?œ;pYßc`?–Äó©ISË?ïhZîý½õ?~ªø‰
¢"?'ô¢(ßGN?~ªø‰
¢"AGN4FGL J1359.1-1152?ÔOp³ÞÌ@GՊ"-QrÀ;ًŸeÀ<ÏÅ'iú@#"ß³Y^@?çK¶ý'¢1?æZŸRk2?ã÷{a .?øȃweR@ùi'é÷Ö?ïñZJÏ1¿ÍÏã؂µ¿ãßIÈ¿äøRAkZA¿ÿâm•Q?ÊxýrñºAGNbcu2MASS J13592131-1150440?ïúyÛZ¦Œ?=°ÿk¢fÐ?F'¯ÍÂ?=°ÿk¢fÐ?ïî\áϵ­?o7â›qZ=?a£	γs?o7â›qZ=?ïj!›S?€'aÞäFÒ?‹åxÅW›D?€'aÞäFÒ?ïú"" [U?: ŽÍäßÑ?E­±qí¶Á?: ŽÍäßÑ?ïóM·?]%^ñyŸ?Yeø‰E…?]%^ñyŸ?ï¼íÙYDŒ?‡@'ѵP?€Ä‰š•?‡@'ѵP?ïtݪ$ô?ŒIéème?'dJ»ŋ?ŒIéème?ïñLôón?`J(ßDŽ?]fü1–w?`J(ßDŽAGN4FGL J1359.4+0202?ì<'
öló@N'¼U†DÀ:"R:_w_À<Qhª
…@ ¿'țæ@]¨!ò™?Ëæ	³õ?Ï؎!yd@¿2½ÂmÎ@Z½Ä³Ï?ïÎÃè!¼é¿ä…Õ"ܤ¿çuM‰öŽ¿áÉ/ß@¾¿ïÿ×,uª?æ9i"ƒb¡AGNfsrq3FGL J1359.2+0204PKS 1356+022?ïöTÎ
""?MJæD¤b?SVcäÖÙÁ?MJæD¤b?ïîOÔÝ+?hZÜc{w?a°*ëìË?hZÜc{w?ï²ÝMe?y¶=–s?ƒH»ðƒx¬?y¶=–s?ïöy8G'†?>©ÿ£H?S
"˜âê?>©ÿ£H?ïøÕ)pDi?JҞ`ß|?L«Z%¤nF?JҞ`ß|?ï©ë&æ/?—­Š™ë?……6IãÚÎ?—­Š™ë?ï0."UmM?'è@8ã«?™ú/sšˆU?'è@8ã«?ïÇÍ-°?kLWEEL?|rÆÚç?kLWEELAGN4FGL J1359.7+4012¿…ø͞¾M@Q°–»™À:V²w¶ðÂÀ<|J{NTø@^VòU'@ž[BEõ®?ÂZCBð?О饴¦@	<J@•òE@G,íHî0?ï÷6Íòfº¿Ù«"}¨¢K¿è>Æ¿—…¿ê~€¿ê'•¿¿ïü€s,óAGNfsrq87GB 135731.7+402612?ïëñHP7?a݃Pœn?d~¨'
?a݃Pœn?ïñò½™
?aš'"G9_?\…Ù'?aš'"G9_?ïMó}æ‹?'›SÆR?‹ìƒ.DÍ??'›SÆR?ïÛõ"Q?Y3-®"?r=îÙU1?Y3-®"?ï×rñËE?vSjœDˆ?tF†ûpôì?vSjœDˆ?ïÒÊö†?wø6¯'ï?vš"ã@Œü?wø6¯'ï?î('à? ÕAá,óW?­}†ïl
Ê? ÕAá,óW?ï\düII?€É,ÎÑôÿ?"s`xOlÜ?€É,ÎÑôÿAGN4FGL J1359.8-3746¿îÀÞÿ¡­²@7&=_ÜßjÀ9…/…(ÉÀ<¨a³y@ºYÀ7@"ý°šg?¬ªþå´á¿ 3ÀîÈ?ó@YÂ5g@N}âÝ?â{8 Z}û¿àr·!ê¶m¿årÚ/­m¿Úx›)ñì¿ÚÄGÃ
0j¿åÅYa›AGNbll3FGL J1359.9-3746PMN J1359-3746?ïþ(¹ÔïÓ?op7{S?-t`9ä'n?op7{S?ïñxÐm¸?a.6¼4?]^®\Wm?a.6¼4?ïøô¤90?=¦ËLt£?L/à´½>ž?=¦ËLt£?ïüE\Þ0?'vŽÀþ è?=ÕVøǯ?'vŽÀþ è?ïýwEmÉ?)*f{~í?4EÕÈzJ?)*f{~í?ïÂ3–°['?"¬ñM%Eá?~æ4´àðb?"¬ñM%Eá?ïø2‡lì?V£†?àñ?O5ãqÿÑ?V£†?àñ?ïõ@eîå?Dù(¿I©?U3¨(F©?Dù(¿I©AGN4FGL J1400.2-4010¿í¤ÃÓÌ<Ñ@4Ðù;À oÀ;ñ՚ѨÀ<Š¹æ@;Y@ ÐXz•rn?ÿ"<jÿR?ÉèxyäG"?³ÿè¿,âG?ä¢ÿñ?ïäOþ΅<¿Ø—"{ªñ0¿Úki¦Wî?ÞçÖyô¹¿äh M¼¿Úd¢Qy¿á'Y
]QAGNbll2MASS J14002208-4008235?ïü3o÷'Q??ÞeO$\?>dˆ«J??ÞeO$\?ï•=
ᅪ?—?Ç_ä?Š°½D¥?—?Ç_ä?ïÖé#x2Ê?tÏëgЯ?t‹n%ª?tÏëgЯ?ï|´!óŒ?y¨G¢xß?i{à\}?y¨G¢xß?ï÷ùwµø?QԙS/sQ?P
é9?QԙS/sQ?î"¬»	€Ý?·'ò¡ò;?­Õ4Ogò-?·'ò¡ò;?ïÒZ,"©7?{0hØývÕ?vÒé¢í"'?{0hØývÕ?íTøÂôܶ?¤aa­²Ê?µX9çë&Î?¤aa­²ÊAGN4FGL J1400.6-5605¿°;hÙÐð@õ†_*2À9 syt`$À;¥›/›Ï@§ÍŸ°‰ö@
œ \–Ú?µ@1ôCß(?·\<ìÅe¥@,Gõb@i‡-0e?ïÿúŒ—Ó¿å:ú!™­¼¿è.[}T>œ¿äǸ@MÍé¿åyÁg‰&¿ïÿܞüÚÝAGNbcu3FGL J1400.7-5605PMN J1400-5605?ïý]8óÅ?-kÜ‹Ul?57ÑÎ8Ö?-kÜ‹Ul?ïßBҞ&?z¤®
1?p^ö OÕ!?z¤®
1?ïâ'ôM?gsœ6"Yí?m~姦Úð?gsœ6"Yí?ïú)
·Å÷?1ç€ßð'?G[É¿ÉFº?1ç€ßð'?ïþD'?)~^2´M_?.Ë´ˆ¨?)~^2´M_?îø…P†?ª™¨ß¼üf? §®nãš?ª™¨ß¼üf?ï³5J,?''î'9?ƒ2¸çK(÷?''î'9?ïèÀi:	?V¨ F!È?g?ÿjÊ÷O?V¨ F!ÈAGN4FGL J1401.1-3717¿èuehd˜@7†Qm°ÝƒÀ:ˆWUQk-À<T"ÿ®¡i@ ÆK¢ë§Ù?ýJm\#íE?ѽH WÎÉ?»®ÛJ>´?ìÆÝ¿¹=ú@©ùŸ"®ž¿äp]€c½•¿äÐvH¿æ•§œ'œ¿È/Š1FÉé¿Ýê …0«ï¿âÞë}'üAGNbcuNVSS J140113-371757?ïýæCQŸ–?"™`¥©Û?0Íä»dý?"™`¥©Û?ïïyÜ 8?aèתÙU?`†#¹LK5?aèתÙU?ïôØ
êñ?V@ÊÊbë?VOä^UW?V@ÊÊbë?ïö}õ›šr?9n¸›v?S+¿Û%?9n¸›v?ïþQml%S?#e$$¹X?*é&	nu?#e$$¹X?﹫.0XÒ?ƒ[I¡Ã|?•4oW?ƒ[I¡Ã|?ïøŠ{Ë?aB!Ñù"Ñ?M×ÆcÝ?aB!Ñù"Ñ?ïÏü]šK,?iñPüþ?xÑQÆæ?iñPüþAGN4FGL J1401.2-0915¿í°òÚ0@@Hïâ£Î¦ÂÀ:¢nÚ©.bÀ<''¤{u@Í>¿‰È?ÿæ҂s"?ƪ4Üօ2?ɗ(¦w!?þó(ýOL@ë8[犿ìî`e›eL?ï÷`Æu¿äò–UAzõ¿ÜPj{žÝ¿ë±Èd?¹w?§ŠÈñAGNfsrqPKS B1358-090?ïÚmï>39?qÜäÏð ?rÉj…Kƒ?qÜäÏð ?ïä8Hñ¶f?pl)–HΝ?kÇ·>d!?pl)–HΝ?ï¥f™œ~?ûCLëÍ?†¦Y˗Pf?ûCLëÍ?ïÒãZéì©?]ÄwA9?vŽR‡šL?]ÄwA9?ïK'xä?œ"w¤&eo?œývˆ±…?œ"w¤&eo?ïu`]wL?ž ŒáX!?'Sý'™H‡?ž ŒáX!?íÙìºÖu?¢¡0Ž3?±0š1o
Õ?¢¡0Ž3?îþ#½°‹_?ò·ºc`? Ä!‡®?ò·ºc`AGN4FGL J1402.5-1827?Û?
#fÙË@D¡¥q"À:($5inYÀ<(]yWÚ²@
«)¹ã@·Mú^ÖO?½¢³ôŽ²¶?rõoÇýÊ?°öÌz—uÓ@¼"K̲ ?ì×aPQý¿æŽÛʖ'¿ã˜íl…¿çŌÁïÏ¿ïÿþó…õ?ïÿÚ €AGNbcuPMN J1402-1825?ïì»ÃÌ.S?e™ú£°Úå?cD;ñÙ-Ò?e™ú£°Úå?ïóm;93?YIßâ5i?YÉ%ùÆ?YIßâ5i?ïeªýwÃ?M×*G?"J QžI?M×*G?ïóPg  ‰?IIuqs™+?Y_1¾¾í?IIuqs™+?ﶴCáM°?ƒ©=nÕ«?'Rîþe¢!?ƒ©=nÕ«?ïÀÉzC#Q?"™yZ¬@]?›BðLO*?"™yZ¬@]?ï"ü
?–T½Ó|í¦?œ
`jíÂb?–T½Ó|í¦?ï¶f@Ѭ[?yÜ}¶…?'foÐd]U?yÜ}¶…AGN4FGL J1402.6+1600¿ë<aÿ	Ç@Q†	€²BÀ;-Ãք´À<­póˆ"@ …H~Éà?ÿj`Æê4½?Æx"%çEI¿{)øã0Zt?´¹øå¬Ã@™'6¿ïÿçÁŲ§?ïÿÿ>¹ú¿ëbrϏ¿ÅÚñéû%¿Õ0ÿ;ßÕ¿ç£ìòù‡AGNbll4C +16.39?îKhøÖ°?É<#S¹‡î?§IqN|?É<#S¹‡î?ïóQ=å¿?i=æ1Ñ?Y]ßG»bè?i=æ1Ñ?ïRz˜™â?šÎyVJgí?Ÿõ°©}'Î?šÎyVJgí?ïû²"xƒ±?+2ï©ííÀ?A5¯Hÿ»?+2ï©ííÀ?ïùv½1à^?U̐|3?J%£²WB?U̐|3?ï¸MQ [?%©ðšUƒ?ì«Ÿ3—?%©ðšUƒ?îÓ
ñö|ô?ž¾‹sÜ´?¢ÏPÞàb»?ž¾‹sÜ´?ïð_÷6'É?TQý'³Y?_@F.†?TQý'³YAGN4FGL J1402.6-3330?äŽêž;aL@;GÜ7£ÛÀ:˜) ã9÷À<kiA@®[®ýY@:9Å«â?Ò¸µ¾"N&?ïj-›C¾@	¼=h@[:@1mD&¤?f¾uœ¿¨»¶OùC¿î!3âÂ]¿â$A"HFÁ¿ïÿ••_x?ìѹÁ,Z§AGNfsrqPMN J1402-3334?ï–±2'y?™Þº6Òaþ?Š{S¥œñ¹?™Þº6Òaþ?î«,5ŠrØ?±ñýÞ½?¥M<¨4¹†?±ñýÞ½?îÁTÀï?"›žn¥?¯î£ê³ñ?"›žn¥?îUòº¿{x?•ò"S?ª ÔRPz"?•ò"S?î
jô7?¶ö]&±!?¯/P¼Žš?¶ö]&±!?åI=`´?Ð}Ý¬K¬?ÕÿÕm…>™?Ð}Ý¬K¬?ëƒ%Øñb?®Õö¶èûP?Áóhœ:w?®Õö¶èûP?áð²÷Ë?Âxm9"KQ?Üéèšk?Âxm9"KQAGN4FGL J1403.4+4319¿æN©Œ3ˆ @Q
ðoiDgÀ<#01 3|À=$P%"õ@"…–VÄ?÷"Âkðê?×û .y?ÍЛ¹Y}u?ù´@€#@¼&‹*‡¿ïÿý{ÁA~¿ïÿÞ°ô)?ð¿âH+üÆ¿ÂDm'ºZ¿Âd5^±'2AGNbllNVSS J140319+432018?ïût€?M¬?Ë0˜?B.xb?M¬?Ë0˜?ïóƒã'á?jcñ†ˆw`?XùÀs®å?jcñ†ˆw`?ï¤&²55±?ˆ·RòS4ª?†öShc¿ä?ˆ·RòS4ª?ïø^Š}?AÊV™ª>j?N‡¾­tïñ?AÊV™ª>j?ïûê¾i š?JU,œ´Ü?@U	6¤Ò?JU,œ´Ü?ïÕ4…×b?¤ûw-&µ?ue½zCšä?¤ûw-&µ?ïàŠÄ¿?üSÏÀ/?‹ÇÝU¯T¯?üSÏÀ/?ïçŽÓ~(
?d;kâ	s"?hq,°'¥y?d;kâ	s"AGN4FGL J1404.8+6554¿œÊ÷ŒH@HÇé·¿ŽÀ:ªøf®‹À<Ž~(א@>Â?Ö?ýÕ%t-Ï?³š³Êó-à?«Æ¥bÇí·?ö7yU@
uèúÕÉ¡?ï÷€—9î¿á"†?IÁë¿ÙŸ:":½k¿Ü‹‰`'eC¿ás°0´Ó²¿Ùl#"¯¥AGNbll3FGL J1404.8+6554NVSS J140450+655428?ïþÞh'Êÿ?®)TØ?"shµO?®)TØ?ï÷² *ò?QÏ[è÷	h?Pšäùc‹š?QÏ[è÷	h?ïö;>²?dã¢Ñω¡?Sˆý½¢Õ?dã¢Ñω¡?ïø–|ƒ´*?5"P
•?M¦S­ÿ?5"P
•?ïþAÁbص?|ê,Ë7f?+ãìĸŠ"?|ê,Ë7f?ïÝDìÄ?s/§"á?q]‰¼iû?s/§"á?ïø#̧§¾?d¿hS…?OpÌ«õ¨Â?d¿hS…?ïóå߇(m?EEìDZ3J?X4@ùî6¶?EEìDZ3JAGN4FGL J1404.8+0402¿ãZVb¸@N€ƒ§ŸíÀ9éF¹!õÀ<MÁ}ä1@…$1–¬@b"òB¨?³pbé"='?ƒ\³VGú?Ò'!,öX@Qî4P"˜?ïÂ.]á\§¿Ž¬)ò N¿æù­5WС¿Ò=ÉD6·¿æá	/Sª¢¿ÒºBUeAGNbll3FGL J1404.8+0401MS 1402.3+0416?ïý¯ãÝàp?'»ÇO<ä?2€áƒUâZ?'»ÇO<ä?ïñÔhD‡?_nLJÆ¡´?\W/\|O?_nLJÆ¡´?ïôE¥YHú?]\,sÌæƒ?Wt´ò¸\9?]\,sÌæƒ?ïñagñM?JýôÔÕ=?]Ñ=KšE,?JýôÔÕ=?ïûå"ü%?;"ϱªÆ¶?@i¯|,¤r?;"ϱªÆ¶?ïÈX«\?ÚSÁRƒ?{ÓûÁŠ*?ÚSÁRƒ?ïííO½ò-?qڭ₩?b°iéJ€?qڭ₩?ïەê"åû?dnðR'à?r5
ßér?dnðR'àAGN4FGL J1405.3-0640?ì
ҟ}<@IàU!š"{À:ð¢nTqqÀ<…e®°'@qÛ$(~N@…ŽêéîF?ΠiA#?½ÆŠdó¹?ñ$lü'œþ@tP+çd~?áC"Lx?ïëقgÎÆ¿êÑ¥CñÇX¿ÇJ|ùzÖ¿æä_æo‹¿ïÿ'Q¦»ÁAGNbcuNVSS J140504-064056?ïûkrâ.?>¹\›q?BR4'*
?>¹\›q?ïӑÔö‰V?yÀ•U4?v7sI?yÀ•U4?ïÜ®õ©îY?fÈÄ}¾‰Í?q¨…[g"?fÈÄ}¾‰Í?ïÃ"
¾Q?cŽž_òD?~nùèƒÔ?cŽž_òD?ïòÈdæ½?YWãs'É?Zo6HƒRä?YWãs'É?ïn©>Zâ,?™¥V>º ±?'*Ø14x?™¥V>º ±?ïÀ…
<öÎ?'yâ4,'?½yC÷õD?'yâ4,'?îÙض1w>?"Ø€w?¢btœ¥%?"Ø€wAGN4FGL J1406.1-2508¿ïÿ²Sézò@A[¾ãÕýÎÀ:Û»}0À<Vºlwø_@,¾yø¿?ÿ–Ù æ?¹'ßV?³RæVáŽ?ùˆ
%ð@
¤íÛ:MÚ¿ïÿ'¥4?ïÿÙiÍy¿ÚÜÜåHĕ¿ÜˆÖž椿æob¬c¿Ö§ayWAGNbll3FGL J1406.0-2508NVSS J140609-250808?ïþªŠ$( ?K®Mn!?%Wa5åÊé?K®Mn!?ïó:Ø/w?\_†2?YŠOYnƒ.?\_†2?ïêÆÁî?v¦§oSHŸ?e9÷Ð`?v¦§oSHŸ?ï÷/Ä­ˆ?;uÙý‰]?QýŸò³ð?;uÙý‰]?ïþ6\'&?'îi¨@W?,š:r`×?'îi¨@W?ï«iàÞ?"; Ü+T
?~ª} •?"; Ü+T
?ïïùöY@Â?n@™»?`	ä˜6?n@™»?ïå›`vÀÚ?^+T)ëfa?jdŸÜ͵?^+T)ëfaAGN4FGL J1406.4-1654?åùg3*@E,ÔV.	ÿÀ:à翗Z$À<eôA…ÜM@v‰Á_[Z@_±@L?Ææb H¤?%U`?ìæ?ÇåTƒ™@퇂k?àM³¿ÞIMü¸!ð¿à+bùÌ	¿éD5囹¿ã»gêÊ䕿Ë58›ýÌõAGNbcuNVSS J140638-164954?ïýÑ2üÆS?%*kÒΦç?1vgÍïž-?%*kÒΦç?ïòI,³?`zæ&@U¸?[m¦àu¿S?`zæ&@U¸?ïì"¾i2?[HƒßIÜ?clï[~q?[HƒßIÜ?ïú`'»u{?.+všƒ?F}õŠ•t?.+všƒ?ïú=÷eo?CçÚQ]?G"Љ9"?CçÚQ]?ïÃÌÀã_‹?'ÿ/þ¦à¾?~Ÿ«ÜÞ,?'ÿ/þ¦à¾?ïÕþ MN?{½?Ú?4÷?u¹5X¸ç?{½?Ú?4÷?ïæÿ˜Hƒ?XרûÑ|?ig±ý'?XרûÑ|AGN4FGL J1406.6-3934¿Þ± ‡<¨[@5z9'ÍÀ;2Êo${
À<œ!Äuæ@#14…×b?óòPµû?Ö|¦Ä¥`ø?ÜL³aì¯@ß덂4"@
^6¬j—¿ç‰Ò¡ÍðŽ¿ç/<B¦¿æ`ï. ¤»?Í#£×dÖ¿")xc,äԿϊ"=fèÂAGNbll1RXS J140630.3-393508?ïþv£¨ï«?$Ô©—a%ð?(•ÁH±.?$Ô©—a%ð?ïë½»n?iü6tî­à?dBE$maÉ?iü6tî­à?ïÆÆÜP€ÿ?}>(qµ?|œ'ÇA`[?}>(qµ?ïÿür¤/?™²ý»ì1?àsÑ;¤ú?™²ý»ì1?ïÿK@+zh?R*aÜ]Ç?—÷[•p?R*aÜ]Ç?ï‡g?ª9û?˜ˆå
ب?Ž&0ÀU>?˜ˆå
ب?ïՑéÁž?~ FñÿÕÄ?u7Nü‰?~ FñÿÕÄ?ïüƒÐžW]?8awÿ56?;á{Qpˆf?8awÿ56AGN4FGL J1406.9+1643?ïÉ='@QjŸDÔEÀ:·í£ùoÀ<'"ͧ¾ @ ÔÇOŠVÜ?øÒó*öN?˅'òP¶?Ì£f÷ÛÄ6@³Þ¿=˜@³ã»¦´µ?ïÜÛ7ɚé¿â} _žû¿º¢>?¿Ðºèß'q¿ÛdóiÅ¿äF a3÷AGNbll3FGL J1406.6+1644RBS 1350?ïö`#×·?U Ó	©ÙL?S?·Ö¢­?U Ó	©ÙL?ïçí{²Â¤?r//ßëßI?h")kî?r//ßëßI?	Iï|?Œ¹'g·?‹ý·Òôí?Œ¹'g·?ïºEò0<;?c@½±è-?nƒr9#$?c@½±è-?ï÷³×C¯h?X	6sÓ6?P˜P÷oßË?X	6sÓ6?ïyóŠaÿ`?¡"õ"?ÁŽ¬àÜ?¡"õ"?ïo¿JÙ3?'s\¦Æ")?'¤Ý¡?'s\¦Æ")?ï<®Á˜Å?†t=ÉÍ¢?˜j?0cí]?†t=ÉÍ¢AGN4FGL J1407.5-2706¿ì´I× ¡‡@@a輜$À;oŽXøÀ<¨¼ÆÅKÏ@!jÑF"@Hpa'ëO?¡6›óf¿º'ê?Nt'?ù"ÿü¥?ýôc>¾­?±f£M!›Ü¿î苤äPw¿×0ÄÃéÏ<¿×êäûAÕ7¿Õá!îgQH¿ÇÚÄ\:éAGNbllESO 140425-2655.2?ïü"j¹q?3ˆ.v¦îÄ?>ì©êÕ5y?3ˆ.v¦îÄ?ïà"9,"Ô?rñ©-¾Ý©?o{ÆÒSØ?rñ©-¾Ý©?ïòµãùg?_¥&)ZMq?Z"9y›'ß?_¥&)ZMq?ïòÞÎúEù?Lo†È"?ZBaäømà?Lo†È"?ïúαd¢¨?>]EcÑ?DÅ;L¨Ë&?>]EcÑ?ïe+­¥6¨?¡!R™|?"ZŠP€"ô?¡!R™|?ïòÕZ::?k)óSRB?ZUKs2]?k)óSRB?ïY5q¸b?`"¤Äi?"ÙQÌm¯Å?`"¤ÄiAGN4FGL J1407.6-4301¿ï¬Ïô'7@1°§¨PÀ:Êõ\8À<B¾Ü-"@ߗ mˆÅ@Vç_ö	Ý?º‰ 'RTa?®`ÈAͪÃ?ò$ötfj@)¼=]ƒ"?ïÍ€°ên¿×.¡S!e¿ßÁf<J7¿á›·¡Aƒ®¿á'€ãÀ.Y¿ç*`Æê4½AGNbll3FGL J1407.7-4256SUMSS J140739-430231?ïþÅÁHh?ö_–Tj/?.#¥´ß¹?ö_–Tj/?ïëûؗÊü?r'¯ÒR?d''Ð+™?r'¯ÒR?ï÷#I\Y?T›¢§òK?Q¹ÒéVNK?T›¢§òK?ïþ&O[C.?´ocP*?-›
u
·?´ocP*?ïýÚ?=?%ñp++üg?1/L p­D?%ñp++üg?ïŽ)§ ôJ?™jñlg§ò?Œu–&"á›?™jñlg§ò?ïõ	K¥'C?fD»RõBÿ?UíhO'.?fD»RõBÿ?ïü‰¾$?-ºO1ӌ?;·È}—~?-ºO1ӌAGN4FGL J1408.9-0751?äAó9•o`@I%ñà'Œ7À8³çïhHÀ;Ls¿ë<ú@ÒèŦ¾@¦Ós¯û?¨g^«Sx?²ßß#;™^@	™>›A:@›¯|¿©Ý!-ÍË¿áFvÜÖ/L¿å¦@q	W˜¿å
ñú´g¿æºy
2ª¿ëyÍ¡^	 AGNfsrq3FGL J1408.8-0751PKS B1406-076?ïý½W j?&H¬0:ð?2‹í	ú·?&H¬0:ð?ïòS,€o/?aE0mŽT?[Y¦™m3?aE0mŽT?ïà%D24?r4íŽ<?oÚ»«oãp?r4íŽ<?ïþ"臓]?G»$ÙÌX?'±w'ý?G»$ÙÌX?ïüÔÿm«L?26Ó7Ø|+?9X+ªTR?26Ó7Ø|+?ïÀ¸O+%?ˆ}ç³"j?û£êHeL?ˆ}ç³"j?ï½Ç
b{î?''…³'E?€Ž=^Éþ«?''…³'E?ïû4{»?6%ŒJ8?C.Ñ~ã?6%ŒJ8AGN4FGL J1410.1+0202¿ç¯nQ08@MO@Än&À9Ób ß9À<V/Ñ|_@ÖC€Þ6Ø@óò
s÷I?¶ôN›ï_I?· Täl|?ÿ‹…L»@
ùÇÚñS?׀ät^Í¿å)B™'¿ãï°A{ËR¿Þ{†^(P¿ìèné¦ٿïÿõ4ÊãAGNbllPKS 1407+022?ïøn²vp†?CØHN*µ?NE5×µº?CØHN*µ?ïò$n¹
?]¹Îª1ì0?[·"±§Í¥?]¹Îª1ì0?ïŽ0Q×c)?Šû¢KŒ?ŒsëŠ'5Ï?Šû¢KŒ?ïò¨q¬HQ?EÙ4,Ýi?Z¯Ö*¶?EÙ4,Ýi?ïô†PLÚµ?Ou«©±?Vó^çØö?Ou«©±?ﻳ˜P÷È?…p'SÁ?ò¡F?…p'SÁ?ï¥Íпö?‹-ƒJ?†Œ‹É_JŒ?‹-ƒJ?ï×4jüßJ?c!ÜÎi†?teʟþ¥?c!ÜÎi†AGN4FGL J1410.3+1438¿í¿f‡@Pòy»­À˜À:aps/¢…À<[IŽ¿@Vp–ëêI@ߢ'g?Àe@ ¬s?¼ÂSL-U#?ýPÕ©²ì@`dÚEÀ?àý®(`q¿Ë¬Þð»¿^¿áƒþÿyó¿á¥?à?Æ?¿âlÁâ
&¿ç€[AGNbllNVSS J141028+143841?ïõ³ý·À?h"ëûk?T˜å¶1d?h"ëûk?ïØØõ¶6D?'Ä'<šdl?s"…+**?'Ä'<šdl?ï·ë9}ç?…Øç>;?'1§ö´<?…Øç>;?ïaz‡–Èë?rƖh"è'?"ЯÞ°ž?rƖh"è'?ïܒï¦8?x±x²h"?q¶¾ô?(?x±x²h"?ïnׁº2?®|ƒ-×?žò%ë´?®|ƒ-×?2ei"?KøÈ?^óUw«³?KøÈ?íb
ºÕ9¿?™7»Þ1?´ïª(zK	?™7»Þ1AGN4FGL J1410.3+6058?ïå;Ӎ'¾@JÏäy'¼VÀ;ø|²F+À=* ë2¢@"o±UÍè?õf|¡;N‹?ÙS¸ä¸{Ý?˧À£ÉžD?ó0Ì5Î&@‡¦<•1«?ïþ—Ô¿ïö({ILz?éÙl€OF¿±R á·j¿Ò|ˆÛ—¿Á7»˜œïdAGNbllRX J1410.5+6100?ïýÅ;š0?0…ѱ½ë?1Ö!¢o¡?0…ѱ½ë?ïöx*;Æ]?TØ>Î"‰?S«¹í¥?TØ>Î"‰?ïÑô^·‰?|ôÙ0µa?wд@ïs?|ôÙ0µa?ïü–Ö"•?+t½ÁÓv?;IKÎ¥ý]?+t½ÁÓv?ïÿS~¸?Ô£o'ºâ?:ö#±ÿ?Ô£o'ºâ?ïÞn¤'4å?qÛßÙ¨«?pÈ­¢÷ч?qÛßÙ¨«?ïÚ`Dýú±?z‡Ùœ¡³Z?rÏݞKZ?z‡Ùœ¡³Z?ïû•†©@Å?:žÒ³Jγ?A©äT4e—?:žÒ³JγAGN4FGL J1410.4+2820¿é[hd©‰@RÿCAžÀ:•ÝÞmAÀ<£xOYÚ@ï£ö¿ºk@
·Üz¿º?ÂpPJUl?»œzŸƒh€?øÂ^™éJ²@#JæX9?•"|¯‡¿Ôs£eË5ô¿ßéIDÂ|½¿Þ'G۶ʂ¿æ3OîTÜÑ¿ï´
ɇïAGNbll3FGL J1410.4+2821RX J1410.4+2821?ïüؖ·ð?2•(×
;ÿ?9;Ojg¶²?2•(×
;ÿ?ïóýLÇY?bÕVìÈV ?YÐX²Þ4?bÕVìÈV ?ïì¾*ƒÈ]?d¸"&ã?cAÕ?¾ƒ?d¸"&ã?ïŞˆt`Ù?_=%t‹œœ?}0»«²‹Ü?_=%t‹œœ?ï÷ÛߗÞ6?M¯߅n?PH@äT~¯?M¯߅n?ïÁ•vŸC¨?‰RD›ev§?5DµÝŒ)?‰RD›ev§?ïÝ0HXo"?x€Èöª?qgÛ¼jÞ'?x€Èöª?ï<¸$Ÿº?
Æ}ý=?˜hûfõÔ?
Æ}ý=AGN4FGL J1410.5+6215?ÛÚ"BB@J@8ÅCÀ;k
Çhß½À<»§œ'›ž@ŠK—Øú-@47yéÑ?Áe»È®¿º·¢™œ?ûz	Ì1œZ@´)Q.?ïÿƒVR¿çÞQ"'¿ãŒÝÞíᚿåÉ3 @|È¿ßÐÜH*¿Ò/ºÏÊ-AGNbcuTXS 1409+625?ïüß=˜¬?-è}g«‰?9Sï¬?-è}g«‰?ïãÛJz2Ý?qL|ø$œž?l$µ"mJÏ?qL|ø$œž?ïڟ>°P&?pY$Èr.?r°`'ÚmR?pY$Èr.?ïå†\"b?WÆ-¬¤£å?jyü·mÃ?WÆ-¬¤£å?ïøá~<ò?LpçX"
‰?Ly½L®6˜?LpçX"
‰?ïÀïÍ?¢V*"
g?œgü»jZ?¢V*"
g?ï}͏ûê?ŽÃƒ:-<?F,QpÇ?ŽÃƒ:-<?îm!×®?Ÿ¯!b¦f?©-îa?Ÿ¯!b¦fAGN4FGL J1411.5-0723¿à'À긽@I3ÞÑ·À:ŸÆh.½ƒÀ<]ùú,h@ ó¿ÕÃk@0«Ü'<®?Á¶f2¿©b_¤3@?æùžßY—?÷Z®Fú»H?ä¥+"˜†I¿§Ež€ð;£¿åø}àU•´¿Ý3žÞ'>¿æ"1l"Ž?"bèyóÙNAGNbll3FGL J1411.4-0724NVSS J141133-072252?ïú"­Ø|?>n*Ì<?E±HK™§?>n*Ì<?ï±}"¹I?‹ÿđ'€?ƒ ¼ixwµ?‹ÿđ'€?ïã
ښQ?r{~9å~?lò%8Ty?r{~9å~?ï–•%Zq?qšÛ ;«?Š`¯Ê+´?qšÛ ;«?ïðr,SC?YsÕVµv ?_§'¶êx?YsÕVµv ?'"(ø?°I®ÙS?§¤'ÖÍp{?°I®ÙS?ïݧÎ	c?yDÕª"o?q,9,é
z?yDÕª"o?ìþ-±?¡0o
Y2<?¸†•tµ£?¡0o
Y2<AGN4FGL J1411.8+5249¿æ§ù ñDÚ@N!uŽ!–SÀ:ÎÜيJqÀ<ÐÒE²'¸@mòGۋ×@'åp1Á?¹ù⯍ 応Oò†qã?â¸îÞðeÙ@
©3)ƒ?ïZTª|?ì¿ä¢ŸÒ˜¾¨¿ÞíC÷Ò¿è~bÁ–7å¿Ì¸éÖrèÖ¿Úa€Îq"AGNbll3FGL J1412.0+5249SBS 1410+530?ïþá³þc?"Hõò‹?!ä¾_ÆFÐ?"Hõò‹?ïø^¤·@/?Q"ù'<e§?N…l›Áؙ?Q"ù'<e§?ïôaö·yK?a'¡v´qŸ?W<I•Š•?a'¡v´qŸ?ïý´­'Œ?iëw2§/?2Z——¼?iëw2§/?ïý»ýœ£d?61tþ»Í?2 FßÝ~?61tþ»Í?ïßk.ûÕ?s,ÛŸ1¯?pJhÐï1T?s,ÛŸ1¯?ïõ&=›0?eo)`ÒúÎ?Ué³Ô€Ð?eo)`ÒúÎ?ïù¬yp.?<ù'Õ¤:F?K™O/áÜ?<ù'Õ¤:FAGN4FGL J1412.0+3836¿ïù,F7¥@Qg¸d"À;†2´ˆ2À<Ž#â]@ ˆÂ%ÔÐÒ?û´{'G–?ÉgöHòL?½ËPËÊnN?öÄçûý<@ì$+#¿ïÿìêy…þ?ïùàÌ^¿Ö ³Ô®C¿Úf÷~0ˆ¿×>?©c;¿èr'~túÿAGNbcuFIRST J141208.2+383521?ïÿYÔ)/?-×Äžö?©‰ÝÚ
?-×Äžö?ïö·JPþ?Xú¼Â90-?Sâ'pÝc?Xú¼Â90-?ïôFÂ1=?Z°ÎgDÛ?WÁs
äx?Z°ÎgDÛ?ïõ=–Ÿ¥??˜ãˆãȼ?Uㄩ…e~??˜ãˆãȼ?ïÿ9Û$Ý?óEÙV«?ßßY—¬?óEÙV«?ïÛy…þ˜?zÞ1}îCÈ?rCrJ7¿?zÞ1}îCÈ?ïñZy"aŠ?hmmÞÙ(v?]K'ˆ|?hmmÞÙ(v?ïàÈxX?`e«½Gô?o7ˆ#šÏÓ?`e«½GôAGN4FGL J1412.1+7427¿íj['Ôþl@DÆ	VÀÖõÀ:¢!óoÏÀ<£èì¾Ü@}s±¨"@‰Ÿ
vá?ºüg>ÀZ?˜Ð—e?}w?Þx~a.ï@­{£ºZ?ÚÙéëÁ"š¿ç E…EO¿âªÜí¬@e¿àyÊÇ9¿èŸú¦ú«,¿Øx' Ï-zAGNbllGB6 J1411+7424?ï¥á…¸Þ{?º	—/˹?†‡ž•7ýK?º	—/˹?ïöŽÆƒ:?RE;Ù¹?Râr¥<›?RE;Ù¹?ïë£Æ²ñ?v=\¯ëÙð?d\95±ŠÎ?v=\¯ëÙð?ïíæncO?Fýß	¢¥±?büe¡±t?Fýß	¢¥±?ïÛÚ…Ø?€iÇ·i¯5?rÿ?€iÇ·i¯5?ïÞˆ)ô_?s±Š"'?pÿ»ßW$'?s±Š"'?ï×k|‹þ?ÆÍ5Pºp?trJ3K¥$?ÆÍ5Pºp?ïÂ×P3t!?e|çwj(?~"WÇYsÎ?e|çwj(AGN4FGL J1412.9+5018?îŒ}~}Uä@OHƒýP"À:õênžCMÀ<²Àsøö!@ê²:O\4@SÌÐþŠµ?蛢Íu¿]Ô³tV×?˜¥w¦Þ.R@	J«GA1¿¦À"üêæ¿èh'Zà÷&¿åBl"4X¿è…y¼"€-¿éKV?§¶¿ïÿ[•R<AGNbcuSDSS J141302.28+501927.4?ïþxR:ú?w? ýHß?(zÜTĉÀ?w? ýHß?ïöëõ&á?V– 1P?R(åóÎê?V– 1P?ïëAÌ y?aíò¿);?d¾3† ¶?aíò¿);?ïúg'È?1ÈÙþ³3?FaÃ"3£O?1ÈÙþ³3?ïþ~-#ò?1¾Ã<ù?.HïÎðø?1¾Ã<ù?ïÞy.Xò¤?tSö,¶Í?pÃhæÄ}Ç?tSö,¶Í?ïãm'd'-?q‡u<³ˆ°?l'nhþ› ?q‡u<³ˆ°?ïæ˜èï˜)?XÕnCðé¹?ig å÷?XÕnCðé¹AGN4FGL J1413.1-6519¿îu=HØÀiØá®aÀ9»1'À8jÀ;'™,ŒP@ۓÜ@]=@ý"$½N«?¼2sÓÝ?™æÇþ9‰í?à.ßFL¬@V†PÀb¿îæÉbµþ?ï"2¼ë®9¿ãbà՘Mi¿á™óÇ™k¿æ)'@¶©¿â"¬Ø:¿AGNsey3FGL J1413.2-6518Circinus galaxy?ïû°±ItÏ?5.Â×`'
?A=;|ZR?5.Â×`'
?ïé$Ê8?s®HÓ-?fàÛÖ·¨•?s®HÓ-?ïãm7»Ù
?pGík/#[?l'Èxa?pGík/#[?ïêÍSZp?RQ¿ƒq?e2¬kւK?RQ¿ƒq?ïâ¡à1zï?hõŒ >#Ô?m^¬(ù…?hõŒ >#Ô?ïV5×t¾?« û¾ æÊ?•?Ù>20M?« û¾ æÊ?ï"@@"K÷?Œ'¢Jjz?ŽïïÑ.'W?Œ'¢Jjz?ï"Ý}§©/?€Š^¶?QÚ?‹ ‹Æà3?€Š^¶?QÚAGN4FGL J1415.5+4830¿ïÑDô¯G‰@O~Ü~ñxÀ9¦tÿ†À<K'5!Iý@Á½CÚu?þDv×ͱÏ?¯z4ú]©©?©ÎЁ6ï?ú#ÝTÚLè@Âƒó•¿åMðMÛU¿à"œÚ–¹ë¿Ýý±¼P'á¿Ýš¿]οà™xa"·¿Þòky˞AGNbll3FGL J1415.2+4832RX J1415.5+4830?ïÿD­ÌH?}ão¸…´?jN2›2J?}ão¸…´?ïöR¬—šˆ?X†‡Rùò?SZ¦GZ"?X†‡Rùò?ïøIgÒø
?HúPuˆ¼?NÚaŽí\í?HúPuˆ¼?ïÿˆÖþ©ê>ú¥Aˆý?
Ê3‰ÛX]>ú¥Aˆý?ïÿ'Ã=ì?§éLཾ?' v"•?§éLཾ?ïÞ,\³Š?u—ÎÁ?péõls.Â?u—ÎÁ?ïøb·Q²È?`;¾¢ÀÏ?Nu#Kq
Ø?`;¾¢ÀÏ?ïÿm1lðª?¢ÌفÎ?YÓõ¨PÏ?¢ÌفÎAGN4FGL J1415.9-1002¿°9©üG¡›@GǤô^À;Ep÷¹àaÀ<Ù¤?åÉ@ÿ0,#@SPÊï?׿-BÖ¿?ïÿþBe«+@"ÚųÔ@¿?Æi†¿ãÍÍlê?Ѻ(»
,ª¿æÁ|^¿ïþaßîé?Üè=)T¿ï^-ôAGNfsrq3FGL J1415.0-1001PKS B1412-096?ïgÖæ"«ž?³ƒU¸ØÉç?"#=bZ??³ƒU¸ØÉç?ï®eýú†? GƒƒIú?"f€|71? GƒƒIú?íKyr)?¥Ùg# z&?µ§›'| ¹?¥Ùg# z&?ïÞ1r$ù?gx¤aŠ½À?pçFð²3´?gx¤aŠ½À?ïÆÅÎX?€ ãàœ?|sƒ†c?€ ãàœ?ì­%h«vL?´Pta¦¹?º–Ôº¤MŸ?´Pta¦¹?ìjÒ¬é5A?¨"9Ï?¼©j˜¶Uù?¨"9Ï?í[ëÀÓ4?²•¼ZoÕS?µ ¡ý׋â?²•¼ZoÕSAGN4FGL J1416.1+1320¿ä±ó²ê£w@PyÛ
Ø0À9ÈÔ¨c`øÀ<X¼ˆ±êÉ@*ËâA(>@*ÈE~R?·h_ºÐ í?Áq}ÝÑØ@¹Ç¼Â"Ž@
{NÀWs"?îB # –x¿ãñãr*¿Ç¿äQ…¦ž¿çÕj*@Ej¿ã×MŸ7¿ðAGNbcu3FGL J1416.0+1325PKS B1413+135?ïúòŽõž?U'·]Úeº?D5ÃG¬Ý?U'·]Úeº?ïì±E©á?r	p äN?cNæƒ\__?r	p äN?4ôÔS?‰/®ÉÞ?‰'2»ë³U?‰/®ÉÞ?ïÉW…Ut?bSҙL8.?{T=QÁª	?bSҙL8.?ïî4'=ËV?f5{ë}†?aËؚY1È?f5{ë}†?ï'R½'¾?™¨Ã>iÙI?k|Æg<?™¨Ã>iÙI?ï[toér?•ÿ)Úds?Ÿ"'k#™Ë?•ÿ)Úds?ï3@20e	?"Ó›gñÍ?™—ù³&ï?"Ó›gñÍAGN4FGL J1416.1-2417?ï\R6ÆY@ATïܜM©À:—#	¼AÀ<e¤m í@ ÑD€bï?ûI
Öק?ÃpÁÂ؂?Ãî•ç2@&º «q@
	œºá<ñ?çžX°›=ß¿ïýf],+?ïæ¥á{…‡¿Ô¯–[ ¸¿á·¾þX
-¿áåàš	+AGNbll3FGL J1416.1-2417NVSS J141612-241812?ïà–·ÖµH?­Þ)ö±h;?oiHo@~?­Þ)ö±h;?ïò`ŠÚ9?`¡ð"³?Zß>Əú?`¡ð"³?ïÞ¢.µíZ?~BC)G‰?p®è¶7_?~BC)G‰?ïñîe´öÓ?H"s·x³?\#4èˆø´?H"s·x³?ïýwéú
?0ç3H;;Ë?7T@Éy†?0ç3H;;Ë?ïÉ
"͍ù?'ßÛ°ßî?{y6ëo—?'ßÛ°ßî?ïág¥î+?yH'`q!?n˜ëˆÌ…;?yH'`q!?ïè/£JŒ/?]Lm†ð?gÐ\ĒÙ?]Lm†ðAGN4FGL J1417.9+4613?Úàï-†÷@P§Ú¤ü¤À:ö¤}"jŽÀ<£QùÇכ@^"JÊÿm@ç#? )?ÆhŠ'¾Ú¿ž"$\"7/?є¨½õo@¬Y=ÞÝÆ?ï¿á—_,¶¿å¶XKñp¿ëÐ÷Ÿnd¿ëñõáõS¿ïìu߀-¸¿ïè(‰ŒAGNfsrq4C +46.29?ïþ1Ø®ò
?1ބãÄ7?,âpï$o?1ބãÄ7?ïõ«*¢O?UbqƒŠÂq?T©ªµ€ú?UbqƒŠÂq?ïÍUØÆøo?z"ÈõÖÊ?yU¢³ˆ?z"ÈõÖÊ?ïî)6bÆ&?OÝrÏ«<à?aÖÉxÀ?OÝrÏ«<à?ïúA9±&©?Oi€é#–L?FûÝïüQ?Oi€é#–L?ïع8µ?wsPÀ®?s£c¹b2·?wsPÀ®?ïÔ6pnö?|fÌäԑ?uäǵù±
?|fÌäԑ?ï…i"¥¾¸?€Áu'TÝ?Ž¥·O±ó?€Áu'TÝAGN4FGL J1417.9+2543¿äÖUÜ_¼@Q¦W>«6zÀ:l–ç7²À<N1©Æ7‡@"Ô˄£=\?õ˜¡Ú°»?Àh3›
-?½âËfÆ2ª@9f1A@Ä3D{-¿î3ᱶF¿ïµ>ì¤Ù?ïÿë""i·¿Éçã(®ÊÙ¿Ár$	ʄ¿» !6ö%AGNbll3FGL J1417.8+25401E 1415.6+2557?ïùó7×ï??Â䚔`;?H3ÏÕ¸??Â䚔`;?ïì5䤖?l×àœxtC?cÊ"ÏŒ?l×àœxtC?ïÜ~b¨ä?uôÕ1Ñ°v?qÀΐÂ?uôÕ1Ñ°v?ï¼D²j(›?pŠ'r‡??€îÓcf,?pŠ'r‡??ïï$ˑcj?WQ?Ð\ô­?`Û4©µÝ{?WQ?Ð\ô­?ïǬKšT¢?"X0ù1+´?|)ÚK'Þë?"X0ù1+´?ï´e–müC?‡/Þrš.ó?'æštÿ#?‡/Þrš.ó?ïIò+I?ŒN8[áß ?–Á½—S,ô?ŒN8[áß AGN4FGL J1418.4-0233¿åã­C£@JÓÙý6÷äÀ8>Ùtzü À;Q‹Ï¬{@Ë¿º?ú<¯c/zA?¤Ê"0'o?´€$þg#¦@Äpë$¦¨@ÓAaRü?ç¾¹ä"¿Ý=ëì:¿×_nû`^¿Ðqal+¢E¿ßÀÒÆӿáO	ß3ØAGNbll3FGL J1418.4-0233NVSS J141826-023336?ïùËJÁš??HJiäÆ:;?HÒÕØÊp×?HJiäÆ:;?ïå;jSÐ?w$M¼rHß?jĕ£BHP?w$M¼rHß?no³°á?"½·‰%|?€œd!*-¹?"½·‰%|?ïò'š³b?DiÝ÷]5†?ZÚË)!?DiÝ÷]5†?ïý¡ÝF'é?(ºŸ7†Sã?2ñ¼?RŒ?(ºŸ7†Sã?ï£Ì?€•ß?šý—""°?‡ðjìH?šý—""°?ïÙ·:ƒ"y?€ÆHÐ.¦9?s$bÊÍ[¤?€ÆHÐ.¦9?ïÜè?]Ò³?`E•$È¢?q‹à2Ú½?`E•$È¢AGN4FGL J1418.4+3543?í¶ö )@QfY_í¦aÀ8'cxu\£À;À®ã­¹â@á¨0¶+@ Á['—?Ÿ¸ådHT?°ídášÓð@ÙÂ~•1@fTȯ1?Ô"g^¿àEí οâøòÔô¹¿àŸ¼ÞÃp¿ã¿''Œ6¿é¨¸á2ŠlAGNBCU3FGL J1418.5+354387GB 141615.9+355650?ïû4ã֌?UO—‡»Š?C,sߑ%?UO—‡»Š?ïõøF<E?YB=}"h?Ts(ÅÙ?YB=}"h?ïãAŸBâ?tS¤‡Š?l¾`}å"J?tS¤‡Š?ïÿµ òd>õ ¾®üû?—¶ÿtüº>õ ¾®üû?ïý"jŽT?.0ü™ÅH‡?6ìª (¾É?.0ü™ÅH‡?ïÖYb"A7?ƒŽpôDm?tÓN›Â\g?ƒŽpôDm?ïçqRA…?x¹†Šw?hŽ­ïõ@h?x¹†Šw?ïÿ¥qéý4>üFÀº?£†?'ü'>üFÀºAGN4FGL J1418.7-3504¿Ûwô®=?§@8xW£UÀ9õ\ŠD'À<+!xö‹ã@qªqX1ð@.…Nˆú?Ã;™‰(ˆ4?Ëz$‰LD@Iæ?@0kؖ/?ãaýKÙÆ¿æšáBO°Â¿ê]3ímVE¿êšn«¯EÓ¿ï VíLŸ¿ï÷6ÍòfºAGNfsrqPKS 1415-349?ïéï!ŠŒ?`&®îÕ7?fþ«›<›?`&®îÕ7?ïÕD¦*Õ?€Wœ<jÎ-?u]¬ì¥4Î?€Wœ<jÎ-?ﱗ'}?w(â_û¥?ƒšÌóŽÝ?w(â_û¥?ï¹®…¨»?h5]îgc&?¸TR79c?h5]îgc&?ï®Ãú?‡ÀmÕ?"|Ø©àõµ?‡ÀmÕ?ï@Û:Vp®?¸GRѓn?—䘰
€T?¸GRѓn?îQ]ã–_?›™ù)»Ôò?ªê/ŽVþ?›™ù)»Ôò?î	KÖm4Œ?— ±Z¾X?¯kBšä…A?— ±Z¾XAGN4FGL J1418.9+7731¿æ˜ŠL8–@CI›Oe™À:^§Å¬GÀ<u¹&&Û6@ fhê¥%?÷ªˆºNE?½ÊèF$ý?Én#Ê	£î@aNÏq@Ñãá'Tý?î!ƒ†Üþ¿Ô?Íà?dÅù1§¿Ì%œq».¿à:aÙ¿àÅþ¢ûrAGNbll3FGL J1418.9+77311RXS J141901.8+773229?ïâHÍñ‡?jC'
âç«?må·1ÀÄ?jC'
âç«?ïßPõïd?t
''ªèB?p~W€8ÚE?t
''ªèB?ï¢{XC–‹?åsë<Ø?‡a)ò‰ù'?åsë<Ø?ï™ÍÓKÛº?jNeD¦˜É?‰Œ‹)™uj?jNeD¦˜É?ïH×ۍt?'qÛEõ`?–ìEփŒ?'qÛEõ`?ïTN¼ŒÊ?£C¨dLU¥?•|ö+Þ¿?£C¨dLU¥?îA¡¾‰Æ›? Ž"Î#H‹?«åäP? Ž"Î#H‹?îÇ2šSu?Žñ¹Ë{.™?£ÓÇ°?Žñ¹Ë{.™AGN4FGL J1419.3+0444¿Öa|$qW@M«=ÈK^À:¹Ïþ°t§À<†ËÈ1]@ ‹ÆGLš¸?ûÑÁ(SÜ?Ñi‹ T?Âxš$W"?ôÈoU"qD?öh\૦â¿ïû9\B 6?ûª0¿ãA؉B	¿×­eL`¿²lTg
{.¿ïü-þ@`AGNbll3FGL J1419.5+04492MASS J14192748+0445138?ïóçíä³?É+H&a?X0%Íõ	æ?É+H&a?ï¶Ý_Ÿ«_?‹ù/ò°
?'H¨
hH?‹ù/ò°
?ïÑ«ä¨i?s]{ßÝü?w~)öþ_{?s]{ßÝü?ïÕØqà\?aJeòüx?uq°bf-?aJeòüx?ïøõÔÐHÐ?YŒáÝM¡?L(«Ê8'×?YŒáÝM¡?îÃ\&$4›?³×+ød'?£Ê=œèN?³×+ød'?ïµ°· Û?ƒ‡òéÉ2;?'"Ò@èE)?ƒ‡òéÉ2;?ï‰()·+?'rÏC¹?žîÚõ¡°©?'rÏC¹AGN4FGL J1419.4-0838¿é_Þ§73j@H-¬îàóËÀ8o‰u_'®À;§™Ûøó@7ë@Iݙ£«?¢XšËÈÀÏ?´':,v«ƒ@?-É@ÒûO—¿ÑµPx…x¿áOY"J¿â¥j­¥j¿äš÷g«
¿æק¼r¶¿ë‡4<G®ëAGNfsrq3FGL J1419.5-0836NVSS J141922-083830?ïüL#ž?16ßD–ˆ?; ºÅð,?16ßD–ˆ?ïòÚÀ!åû?dOÌo±s?ZJQ:?dOÌo±s?ïáבT"D?pCǺ?n(n·ÚSž?pCǺ?ïÿA>Â;,?	ÑÞ4¤
*?Ø.¥)#?	ÑÞ4¤
*?ïýeÍJ‡I?06²É'Ê?4ѕA¥ß?06²É'Ê?ï´Ë6Êñ?þÊÏ0O4?'Í2vík­?þÊÏ0O4?ï䘏¿â?zUeo[†?kgqV&?zUeo[†?ïþLbÈæÓ?!:Ä~ˆ?+9Ï@s<Æ?!:Ä~ˆAGN4FGL J1419.5+3821?çÇï
—ç@QfÙ×À9×À¥wnÀ<=®ä"yw@ùÁ3£'@"ª¼×ŒC?·‰êá¦?ªA… ,I¤?ð\Kv @
ÓìÆè1W?ê<C²\´¿Üœ?¼-˜?¿çßáa¯G¿çç×_w߶¿ç9ö X:)¿âzŠ&_AGNfsrq3FGL J1419.8+3819B3 1417+385?ïþ)>p[»? ú<
õœt?-lã¼Tn? ú<
õœt?ïöa€ÅÛ?Z¥*¼­?Sù<Õ8û ?Z¥*¼­?ïë¤'y?eù¤gBZ?dù[®
N?eù¤gBZ?ïíž{M»?O'‹€À6?ba"n(?O'‹€À6?ïü¾ï¶Ô?6ͬ«p??"	*ƒ—?6ͬ«p?ïݐ|9Œi?}*½!ïÎ?q7ÁÖ+G»?}*½!ïÎ?ïÐbôÊub?|O4J|Qh?w΅½!f¶?|O4J|Qh?ïÀÀÛ/™©?mÑðæõ	?Ÿ'ˆ5?mÑðæõ	AGN4FGL J1419.6-5153¿æmÚµ(ý@!Iz»ˆÀ9W"Iô?ØÀ;¨e­ÙÂ@	$ÕøD @§£Àd¾?·<TÄþLL?´4ƒjX8{?öƨü
,8?ô¢=õƒû"?ÉZB×%+¿âŒ*°­²U¿æ;Þ}yR¿æ~T>p©
¿ç,åÁX¨¿ðAGNbcu3FGL J1419.1-5156PMN J1419-5155?ïê/7k)?d[÷–‡½å?eÐÉ/þp?d[÷–‡½å?í˜õ¡Ï•v?³wtgÇ>·?³8Rð§mN?³wtgÇ>·?ï#‡P
V?'D¤jp?›Ÿ/þUA?'D¤jp?íhœ{÷W?š€ºp@ê2?´»!þëI?š€ºp@ê2?ï«VQ_2?$Ê͉¯C?…*k¯·?$Ê͉¯C?ß^šÅhªc?Ò@oÌpå?àP²KªÎ?Ò@oÌpå?íðn¢ŸýŒ?¡{ 1B?°|ŠèÚR$?¡{ 1B?àuñûŸ7?»þöY|âÃ?ßÁ'þ?»þöY|âÃMIXED4FGL J1419.8+5423¿ã¦Ë[ç!@M&É[ÿWÀ8íL§xnÀ<MäHêT@v"Ž¾@¿–Aö?¢K†¢W>'? –:iˆYÖ?ù×Ì%Ýà@F˜T _¿µ
[b ¿ãÔ ©Óy¿å4°
õ'¿äØuâÛ,¿è!gßjr¿å¿eÁ$øÞAGNbll3FGL J1419.9+5425OQ 530?ïþêŠç"ç?ã¦Ì…Ÿ:?!WSúp?ã¦Ì…Ÿ:?ïø/"BAÄ?R
èw‰_¡?OA®¬çM?R
èw‰_¡?ïórG4
ã?cGUs^ÐP?Yqy­©'?cGUs^ÐP?ïþ·.ï›s?¾{‹`
#?$õ›
F?¾{‹`
#?ïÿ	VQ+¨?¯½Âª| ?Õ5·[Ñ?¯½Âª| ?ïßüï¡°a?qä¾)Ÿ¢N?pˆ17""?qä¾)Ÿ¢N?ïìAzÚÍÓ?pÓ1µ?c¾…Ö˜?pÓ1µ?ïþVF!'9?&QÇçN?*› ñ`·y?&QÇçNAGN4FGL J1420.3+0612?íÉÛ<•÷<@N!	á*QãÀ:š¢Ûa»À<^{Ñ1¶[@9÷8Ü"@®"ø?¼'¡Æ3+¿²Ê'+'u?õ7u'c/@ñ.ÖØ?ïô˜ú7¿à×Nó[¿ëâËf›@¿Þ[*4ï ¿ã«ØáX&¿Ýº¹9r•AGNbllSDSS J142013.69+061428.6?ïþ"0ët?$4Ïuô2…?'¼íúŠŸ?$4Ïuô2…?ïïW_H¡?c…0Ðsö?`¨ ŒÃÃr?c…0Ðsö?ïÚR;u'?{s6Ñê®?r֙7Zõ?{s6Ñê®?ïúˆ‰?00uTƒµ?EßÞÛZ,(?00uTƒµ?ïýcJ¨å?2b'®œ?4å©<)¦Ê?2b'®œ?署¸JL?—õ`›Ÿxï?…™Qíí?—õ`›Ÿxï?ïËIajJ™?{͂÷Ž
í?z[O9¬§œ?{͂÷Ž
í?ïÓ°Q?jh,'AÏñ?vz'Òĕì?jh,'AÏñAGN4FGL J1420.9-7920?èûˆñÀ186†¥À9ÍCÿ3QfÀ<Ќtíé@	6rWá=@±›îÞp?¾Ï8
û?ºRýRü|=?ýs՟Ú%{@Ñ
è èÃ?﫲~lí?ÈJw]¼"¿æ8ÿûÎB¿æÖT5{¿éˆݬ!¿ïûVƒšTAGNbcu3FGL J1421.8-7920PMN J1421-7920?ïó"I+'?QË/]ϋ?XÙl^ø.ã?QË/]ϋ?ïâù·ß?u=«'{®p?mHθл?u=«'{®p?ïÃä"v'?y¬œÈ@Ø?~
øiõCd?y¬œÈ@Ø?ï'
òΔ?q'Ÿ¡YÐ+?‹|¿Q
Êä?q'Ÿ¡YÐ+?ïœîkón?càrñ?ˆÄ[Þ#ì?càrñ?ïžñ&¿Ì?"=Ôò—(ÿ?ˆC¿,9?"=Ôò—(ÿ?îm2˄MW? o¯/?ú?©,ÓDKŽ"? o¯/?ú?í¾ájq@"?›²ÍdB?²ô­¿Õé?›²ÍdBAGN4FGL J1421.1-4614¿ÅßÅ;Í¥T@+¹¼ýKð™À9ü]¦¤DÀ<
rÎ\@®ú²Ž22@ÑÕùµ?º´Fn#t?É	ËÛ¶µ@Aü#Òm@^06Ô}¿à'$,Û¿ÔiËá'n¿ãÕ2ÌÛæ¿ç›xqοïX(ñÿŒ¿ïÿ*¸:n'AGNbcu3FGL J1420.9-4615SUMSS J142047-461431?ï<LB‰?­8ÿn_Ý?˜~–tPRá?­8ÿn_Ý?ïx% L?¦ìñãæ"?û_W4Œ}?¦ìñãæ"?îÈÀ(­%ñ?•ê6únïÃ?£sýq¾ô?•ê6únïÃ?ïZW[JmP?x¨—lMp?"µš!ññ?x¨—lMp?ëEÑD?¼"ÉŒa³à?Â뜻âï¤?¼"ÉŒa³à?쾌uÍ??Àbr=+¦ï?¿rœQ–?Àbr=+¦ï?çyßj\p?¶ÿ"Œ?ÑA+ïG ?¶ÿ"Œ?ëjžOÇú'?¨è×Ñ¢D?ÂU†Àà»?¨è×Ñ¢DAGN4FGL J1421.1-1120¿çr{[–@Fæä:§›»À9ç"UUÀ<>¨È
Æ-@"/¥	9@;û"?¼a؍bÇ?À	WC¡ë@ÿ|í'hs@
¡©7ò4»?ãS¤¢Œ1|¿Þ*߈'4¿äåZ—ü
¨¿äH!ÂG³¿è¾ó…ô¡¿ïêñ°±äAGNbcu3FGL J1421.0-1122PMN J1420-1118?ïùÂr'n%?NX·<V~î?Hö5œ‡@?NX·<V~î?ïí¡2!6?dÖZZÐ?b^ÍÁŁÝ?dÖZZÐ?ïÙr³·ä?ve
KD-?sF¦/³œ?ve
KD-?ïåÌ°?Q͉ýñ,?jíá5u ?Q͉ýñ,?ïÔd—óëä?püÏt?uÍ´ÑÑ?püÏt?﹬3¥?‰8û>è,¬?"ó¸~6?‰8û>è,¬?ï}Ì=Óµ?ŽliƒÓéß?FxJēP?ŽliƒÓéß?ï‹P7G›?w/~,\¨˜?+òQ?w/~,\¨˜AGN4FGL J1421.1+3859¿ÕCٌVm©@P÷27Š°ÉÀ;‹õl(GÀ<_±´B'L@Smfò'?ð´V´A¼?àœBUåå£?ïü{±QFD?øÞÅ7­w@	(ïÀAÏ?ì[Åޜ*¿î·¾b¦¾E¿ÅZè	ã¿êÎ`ÐU¿ïð&¾°ªW¿ïýÚ rfOAGNfsrqTXS 1419+391?ïúÏWÒ¶?\Z­@W˜t?D¡&gçÝ?\Z­@W˜t?ïò¡ª•¹?i±\¶Ç?Z¼ª™ßÎ&?i±\¶Ç?î¥p°þK[?•º8C¿ý™?¥¨ôëÏÇS?•º8C¿ý™?ïÂ7A­ð?p&Øy>µ?~ä_·ØQ?p&Øy>µ?ï÷8ÅL?]˜âɯP?Qۍî·K?]˜âɯP?ïÛü8Rà?w–é¾°Œs?rrÉ¹‡ú?w–é¾°Œs?x'±?˜æf±!æÿ?¥T(|Dõ?˜æf±!æÿ?ïÑÀtyÏz?s0
™"ñ©?wź)G$?s0
™"ñ©AGN4FGL J1421.6-4819¿çÀjŸ—E¾@'Àì1"À:…ñ7`ÆÀ;öp5ó@A- Í›@fQó蚉?Õ½1ø?⑀üâ5@	«f/ßÁœ@‹\¿ô?ï«ÝhüBܿ݉EcŒl_¿êˆÂÔ&¿é²3ž½ð¼¿ïÿøsCÄ{¿ÓÝ¥q"AGNbcuPMN J1421-4820?î¬#Î*4?¾Ø¾y??¥?
À‰§Ç?¾Ø¾y??ëÞÚxÜà–?¼K¿y°£ª?À"–Œ}§?¼K¿y°£ª?îøÙJ4?A}2a¥W?®~Rk\Å?A}2a¥W?í]blíÐ9?–ÇRŠG‰Z?µì™ÛX¸?–ÇRŠG‰Z?ë°ZéZ¢
?ÇC君¡º?Á>"Z•wÌ?ÇC君¡º?Ҁ"©aQ˜?ÑLœE›jª?濽«OW4?ÑLœE›jª?é¯,Óȕ?´	Î>V?ËýCL°Ý®?´	Î>V?ÓðŠ–
\¿?·@r#g?溴úÑ ?·@r#gMIXED4FGL J1422.3+3223¿ïýCŸ^vû@Qh~AN~éÀ9t‡Ù}µ8À<n±lôõá@zæ'Ì@ù©™èt?©úg\'¹?§‰ÎÒ`‹?ùzà…v@·½WÓ|?ïÿù³>†¿ã€!ùO¿æXÞW(Ü¿èwhð?ï¿Úgéek•¿èg˜_ݶ)AGNfsrq3FGL J1422.4+3227OQ 334?ïþª,—?ùaí'?%_¢´-.©?ùaí'?ïø#}¼!?^hÛì'l†?Or	ÔKÖå?^hÛì'l†?ïå‹';`?p)NŽF"æ?jt؟áس?p)NŽF"æ?ïÿãk…ñ,>à¢o "ò>씨|"¼>à¢o "ò?ïþë.?R:j߬f?!M ՅÞ?R:j߬f?ïà»8±|?v¿Ø¬®¼?oDÇÃ3»?v¿Ø¬®¼?ï¿ÜÛ‰?'2'æhA?€É7¿?'2'æhA?ïÿå@6&>ã.9}†é¤>êÀ[µðÓ>ã.9}†é¤AGN4FGL J1422.6+5801?Ð÷«a†ò@K›<Ž%ÈÀ:ސ†Ë`¼À<˜Wk àJ@ Ü}78P~?ö$‰íT+Ñ?ÄÂ'ϨŸ?γõ:,Ü@
›Háa«@I×áRëµ?ÓT^¦ÿ^¿ï'ᐩ0?åôB'KÇ¿¬‹Ü"à¿×éû[Ök¿Þ²'#ƒ'ÇAGNbll3FGL J1422.8+58011ES 1421+582?ïÕè#T?oü¾^Je5?uî€e½â?oü¾^Je5?ï¾²àc¥?ŽÒSm'	?€SzE'fË?ŽÒSm'	?ï‡(zq-?…´œxrâ´?Ž5Ø¡c´Ó?…´œxrâ´?ïrJ¦¤?yþËùÆ[–?'¶«5=ó'?yþËùÆ[–?ïÎuZŽÛ"?qŒ×qœ÷†?xÅR›µ}þ?qŒ×qœ÷†?î«ôÌ´èÄ?·PK$10Ñ?¥@³8!·?·PK$10Ñ?ï/Í~^¼?".0c?š
æU['}?".0c?î5Qªþ­?›î9Ö{ÒR?¬¨
迱+?›î9Ö{ÒRAGN4FGL J1422.6+8150?îÂGd²K@AL\1Y>À;¹$Øý\¸À=\-þ@@©¤æ©Â²?õ'
0Ûj?á4ڂ˜?è•Ú\ØH+@»7^;º?ðuR½g¿ïÿb`ÈAÎ?ïÿ|Ìy?'ëËRÔ¿àÏ8·×rB¿èqgù
¿ïÿþBe«+AGNbcuWN B1426.4+8205?s1Gm?žÙõqŠ›?Œ[#=üøª?žÙõqŠ›?ê½èVU?Â'~"ƒÖ?Ŭ_Þ¦®?Â'~"ƒÖ?î
í2·§?žYïuôAê?¯Q,ÒÍÁ	?žYïuôAê?ç²cÑ¥ht?­áeHú²É?Л8\µ/?­áeHú²É?ïÐ*¿
0?¦QÛHs]Ü?Ÿeú«ŽUò?¦QÛHs]Ü?Ýäw¤ã_ò?Ðùmç[Â?á
Ä-ŽP?Ðùmç[Â?íN{ ñc?¤xDwb¾å?µÜ!®šj?¤xDwb¾å?݆mÂÑ o?½Jܔb¡?á<É—oÉ?½Jܔb¡MIXED4FGL J1423.1+3738¿Íù2dñŸ@Q#_€™À:îؐOÀ<JãÁÛØ@ýÔö¼à?þ׶»%?·«u#I?€¸!Df@	ŠC»@Ò÷BOù?àã;z)'¿Ûþ\;ë¿ÞÀgmÍ¿ÝR•äƒLÑ¿é_6&,ºs¿áš3½œ®!AGNbll1FGL J1422.7+3743NVSS J142304+373729?ïü5¨ƒl\?5øç9ÒÄ?>R½Éš	?5øç9ÒÄ?ïöA&z?Y}Òý™†?S}ÝuAm¯?Y}Òý™†?ïÏ5'‰ ?tÈ"ªåp?xe6λ¿Õ?tÈ"ªåp?ïþnÙ¸©»?¬$Œ­r?)hÈQ¾?¬$Œ­r?ïé;!-?dÆÒð!ð|?fÄޖvÃ?dÆÒð!ð|?ïÛ	Àü"?€à8MÈ	—?rwûÔJÕ?€à8MÈ	—?ƒÏ?EI"ì)?¤ϳ¾?EI"ì)?ïýN¿xê?'ÈbR°$?5Š8 ƒ?'ÈbR°$AGN4FGL J1423.5+4524¿ä;UcLÎ@P'û?¦ßÀ;>eV›îÀ<å'ê)Ôæ@§$íË#@‡±¥)Õ?Äßʇù¿–$ƒºVŸì?Óâ:\È-@K>ôŒÚ?ïÍ8ÝŠ¿ãà'ód¿æ	ˆt®'Æ¿ÙóÿÁ–¹¿ç-ß×kŒ@¿Ódƒ7W…"AGNbcu87GB 142138.0+453705?ïý×Ԓ¾ß?%ߔN†Ù?1AYvÛd‹?%ߔN†Ù?ïöÔî·á·?U'¼®èz?RV"	‹ã,?U'¼®èz?ïøbÓÅö€?<3õ(†ÑŽ?Nt¯ñNÝù?<3õ(†ÑŽ?ïï}õÊ®?BX'>t?`'á'	¸?BX'>t?ïý.éÄ̛?-Ê È'¬=?6ˆ±VÃ¥}?-Ê È'¬=?ïÜ`?Ó!?uÓò~·¾ç?qÏßöÓ
?uÓò~·¾ç?ïõ¥ïü?dtä¯rÃõ?UÀ´šä¸Ë?dtä¯rÃõ?oÝÙ¥?j?2aÓaî?€œ˜'¨É?j?2aÓaîAGN4FGL J1423.5-7829?îÁûç'ÓÀ0x,äd™À:ŸSÌ/îÛÀ<,ƒ2O¥@ö€»|Bq@8xñÝ(?ÇŃ»5÷?ÓscúÑAü@	ÂsBûÅ@Úâ9E›ì?Áùß?>¬¿ä¶Ñü·v¿æ[`Fþ¿ãMf H	"¿ïÿôÕ÷?íx= ™AGNfsrq3FGL J1422.8-7828PKS 1418-782?ïçíåŸ?g&æÞðµ?hó³Ò'?g&æÞðµ?ïñÁLøg?[ã•ØA9¤?\}ÖÂ`?[ã•ØA9¤?ï>è3Áµ?Œ@…'aÓ?˜<"û?—i?Œ@…'aÓ?ïùÝÔ¾?;ˆPv4à?Kü‡þ2ÒJ?;ˆPv4à?ïßy~,f÷?qMâæ±{Á?pC@֎´e?qMâæ±{Á?ïďZÀ.É?‡"ù¯tpl?}¸RÀäې?‡"ù¯tpl?íÀ72qAa?¤ÖB‰•Õ?±þFm¿Ïx?¤ÖB‰•Õ?ï¹t^‡Ûè?v²€œýº?¢è_ÀÓò?v²€œýºAGN4FGL J1424.1-1750?âûWî9À&@CÜÛ7ɚéÀ:³Ú°À<ixX×1«@ œ­çYk?ý&Á½¥?ÃÙjM%Î?¶¥"Ÿù@Y?ô™6Òúä7@
ŒŒ÷¿ïÿ;ÒDÜ?ïüé)ú¥M¿ÛßÚ¾[¿ÞÄÑ ñý‰¿ØI3$Ň3¿á>—jjAGNbll3FGL J1424.3-1753NVSS J142412-175010?ïÿT…Ž?¢Î¯S©?~ÁðIM?¢Î¯S©?ïóLNžYÙ?_/0]ö?Ygb½Ìî?_/0]ö?ïôú3?û÷?^•ƒDû€?V™…‡qÙ?^•ƒDû€?ïþqó7o®?†¯A¼¬e?(àÉTÈ̬?†¯A¼¬e?ïÿYXP?qY&8ñ	?ñÎç¦I?qY&8ñ	?ïËûhì}—?ÈA˜hт?zK‡"l?ÈA˜hт?ïøoyÏ>?[j«wÄ?OâA'Yþ?[j«wÄ?ïûÍ͗'Æ?5d4Yî?@ÈÊíö%?5d4YîAGN4FGL J1424.1+2917?ìË9sX6@Q`ô^NÀ;ólàÓêÎÀ=|ñÃ&[@!mÇÏâÖÏ?úA×:äØ\?Óò۟x€Å?¿ÿ°ÏÁí?ë)À°3å@œÑOŒÊ?仪›I¿ïûÕÎÔ
?ï+Îð"{r¿Ï<ÑW "_¿ä.Äf¿Õ
5ã盅AGNbcuNVSS J142408+291800?ïü<üW p?=‡ô€š3?>‹â&?=‡ô€š3?ïôkì ?[]¹'U+A?W)ÿà¤àÀ?[]¹'U+A?ï×|EBKÌ?|P#&sMÕ?tAÝS+mæ?|P#&sMÕ?ïÉ©Šä†8?dÊî´©Äx?{+:©9ÃÈ?dÊî´©Äx?ïø5~<?PqD½Ö"?O*ÄB½–?PqD½Ö"?ïÙøÙ½m?uÃøËڒ?s",Gÿš?uÃøËڒ?ïÀ¬bÉù´?'ÐXs7ÈØ?©Î·/ñþ?'ÐXs7ÈØ?ï"6Ð:"O?~y±Éi«?‹2Kÿ\%?~y±Éi«AGN4FGL J1424.2+0433?íq€'Æø‰@M3•1ã¨À9ÚÃvõØÀ<(9oV•@Xlþ†c?ÿ®Gx?¶[²Ù0³Q?ÃLßV½&@4±?¨Œ|@­¡kõò?ïGŠ¾4ƒ•¿ØÓØDO:P¿á3§—‰!¿á'­"ãY׿æå>³™õà¿ïÿôw5ÁƒAGNbll3FGL J1424.3+0434TXS 1421+048?ïü·1kC+?7ã	y½ªå?:Fu½-KB?7ã	y½ªå?ïï'¶ÿ?knXàXP<?`þ}v[ғ?knXàXP<?ïǗ""JB?|úŽe®¼‰?|4n¡
KV?|úŽe®¼‰?ïþ5_)Ӆ?ҁQp›Ç?,ª]×KB?ҁQp›Ç?ïüÒQN¯Ä?:ÿwֆÆ7?9muåÄL?:ÿwֆÆ7?ﯝœ¼?"¼¥s¿?"8ÿ_xñ?"¼¥s¿?ïKÊ»€ª?'$²Ï¼?–†¨ŸG¸¹?'$²Ï¼?ïü;±JÜ?,Ñԝª=ê?>"wÌæ?,Ñԝª=êAGN4FGL J1424.6+1447¿Ã'ŠŸb0@PBçÀn¹À:iȉq-jÀ<uÑá߃‰@äk*Í^@7ÆZÂÄ5?¾G\5
"ï?"Æ4=…'È?ח-ä>ÙZ@
ô(Ü¿æ˜\þ2ËY¿äžOv_Ø®¿åÃƓͨ¿ÜTF=Ñò¦¿æÄ¢t´³¿Ý/"—Ú|¹AGNbllSDSS J142436.29+144910.5?ïýÔA5Tv?$ô'[¾—
?1]ø$AIþ?$ô'[¾—
?ïöùTëQ?a\Œ³Û ç?R
X!Þ?a\Œ³Û ç?ïð9|´—³?fÖ¾•ââÜ?_B9e?fÖ¾•ââÜ?ïý"9êB»?"?
bæÙ?3f/g\‹?"?
bæÙ?ïûùcõ"?@‰Wíf"?@ñ.¾,ö?@‰Wíf"?ïÃ!\
×?ŒFø6€?~oQýØn?ŒFø6€?ïñX¤(`?o°Yb"'K?]ÕNŽsï¾?o°Yb"'K?ïù™
z|??Lí©E?I›ÊՈ~…??Lí©EAGN4FGL J1424.8-6808¿ì§Øä³yÀ]{ý§`,À8ÉBÇ$íÀ;€нV@Yà¶Bó@ç>?Ö¯¥?«ç"w³?Ì._6qV@%€Ãÿ@:Š*»À`?ïõáμ'¿ÝU|o?¿æ	àž»Âc¿é#™7t¿ç|}Ê0:Z¿ïÿ/¨;ôAGNbcu3FGL J1424.6-6807PKS 1420-679?ï­¤bVÊ?\ÊjΩ<?"–çn«Ý©?\ÊjΩ<?îÎçFÿ ?©"%Äø§?£‹zB
?©"%Äø§?ì-2TÞK?©<>B݀?¾–mY
§!?©<>B݀?ï\†Í¨Ù—?~;‰ɏ%?"o&P7?~;‰ɏ%?îåI+©7?§š
HmP?¦ñ«li…Œ?§š
HmP?ç±x‡jò?Ê\¢d»¸Ë?Нñ+ô?Ê\¢d»¸Ë?ëF2¾»‰{?­kÂ}z?Âç5Ú?­kÂ}z?èþÎ~A"7?±‹¶yp¦©?ÌÆù³$?±‹¶yp¦©AGN4FGL J1425.0+3615?é°äÂóì2@Qn'"šVÀ9؏AQ(À<
v{‡`@ SEµöâ?û€ û?¶ØÐç
À³?À,2ñÅ«@YQûuVÄ@TxžÍ5'¿ìâT1?î#Cœ7̿ʸÂ~À$¿×`½,à¿à±Šâ¾w¿ßIà>¿jAGNbll3FGL J1424.9+3615FBQS J142455.5+361536?ïðån6òä?\oaqêêù?^5#hÞèc?\oaqêêù?îžcáYV?¯çÖ=ŽÖÈ?¦Áíצž?¯çÖ=ŽÖÈ?ïžáiçÐ3?…»(·8£Ñ?ˆG¥‰{$?…»(·8£Ñ?í"åbg?"˜Ú–‰Ñ?³ßÃw‹G?"˜Ú–‰Ñ?ï™T¢™u?‡aÞg?‰ª×Hj–¼?‡aÞg?êäYf?ˍÁ2LP?ǘoºšg—?ˍÁ2LP?î¬xøþóª?œ¡hŒ?¥8po4Þ]?œ¡hŒ?åá@m#Ó?¶Zfa V?Ô=%é¸Z?¶Zfa VAGN4FGL J1425.4-0119?í¤
}ºô@JÒYÀe¶=À;lœù	À<ÇÏï–ü0@!à*w¢Ï?ö¡›Lø?ف9ÜÆÑ?ߎ0Ú¾R@ŸL{ٕ2@ˆžìää?ïû°&äp¿ïÿùëñ?ïþ¹ä'¼0?li|Š.¿æm›¿8º‡¿ßõ b‹AGNbll2QZ J142526.2-011826?ïûÚY°Óû?Mº&òÜØ?@–šLDcï?Mº&òÜØ?ïì ] J+?nþLrÎÄ?cߢ½Ub?nþLrÎÄ?ïµÜœèGk?€)ê¿?'ˆØÓTŸ?€)ê¿?ïÙ
¾7;^?bI¹Rã¤ð?sy û¼Ê?bI¹Rã¤ð?ïý±>¯pÏ?5b+D-?2vðô7?5b+D-?ﶣ®×"?‹Oºž,ð?'WW.žÒ?‹Oºž,ð?ï̇'°ò&?'ëji?y¼6²…­
?'ëji?ïÉé•Qز?qê Š"è?{5`¢Þ?qê Š"èAGN4FGL J1426.1+3403?àðo&±ù@Q!灃ùÀ:Kñq…À<˜Y¸Øú@zã ùµ@ÓÅåQÿ?»æþ§:l
?¹
Ùͼ5ü?þBu
n@Jzpßf-¿ì
þ‹¶­¿Ö6j?Žá/¿âYÍ "¯Ó¿à™_æÌR¿ã/\äÝdË¿æ@U$õ'ÎAGNbll3FGL J1426.2+3402RGB J1426+340?ïýY"—?Þ?2"'*R)n?56ì>~eÔ?2"'*R)n?ïñR¤âM?bm¯!=ß?][ÐA¦)?bm¯!=ß?ïïŸHç£?l^FÂ"*?``¸#2å$?l^FÂ"*?ïÖõ5]/?X2Tp¯'m?t…9ipðx?X2Tp¯'m?ï÷ã(®ÊÙ?MÐU±Z±?P9®(¤ó?MÐU±Z±?ïËoÜÿm?€yˆ%¬£"?zHiqe?€yˆ%¬£"?ïë) §Í?qûaʝ5?dÖ_‡¡âÐ?qûaʝ5?ïDùL\¶?uDq_?—`Ü›Ó5?uDq_AGN4FGL J1426.4+3625?å[¡TµB@PõöM½ùÀ:Tغ@ÙÀ<F<"¸@/fRÅIÌ@A'Ã'ë?¿
SO³F"?—'(6êÎ?Öˈü@›©×Te2¿âìËð¦¿å:"yÄçü¿ép÷б^¿åË¢Ëq'ú¿á­òKâV¢¿ïÿÀéz-AGNfsrqB2 1424+36?ïûb+w?:%׍Œ1?CϽµÎŒ?:%׍Œ1?ïö'®îÀ?[ÐG¾v	?SØÚ¯àï?[ÐG¾v	?ïé){ñµ\?bœDÂóGD?fփõt>?bœDÂóGD?ïñ÷Ö)±™?Foÿ™Ðä?\Sxb¾A?Foÿ™Ðä?ïðÙ¨Â[?`+G·Œ'?^L®c?`+G·Œ'?ïÔL-2Ç?w¯ÝjŒ5b?uüZsà‡?w¯ÝjŒ5b?ï¼øÖà?'½Uí=?€Áü<«þ?'½Uí=?ïœW»—Š?zi
*ßPU?ˆêR?zi
*ßPUAGN4FGL J1427.0+2348¿Ö
Áœdr@Q
´·,À6Ô{Ås<8À:º¿&¼@` ãzcH?ûHcF uÁ?Žec~võÍ?­ÃŒ #$â@37ÿJÎZ@Á¿}ƒä¿¼Fa
a"¿Ñ˂Iñ»š¿Úú¼#\Q¿Ø"a`î{¿ÞïҋR¯¿ÞÖ-¾ÕlAGNBLL3FGL J1427.0+2347PKS 1424+240?ïóoóÐ>>?gãÕ
1©ë?Y LE´…?gãÕ
1©ë?ïådϞŸy?xÔ '"—C?j›0‰;þ¶?xÔ '"—C?ïN-B‹ôH?"òJȖ«T?–:W©Z
?"òJȖ«T?ïÍý¬Æü?e+I»ÓÛ?yp¯â6?e+I»ÓÛ?ïøþ.¢2x?PúÞ2Е?LE§—#?PúÞ2Е?ï=&?ô|?§Ò¥`ĈR?[6I¢'?§Ò¥`ĈR?ïǪó?‰O%ÒÙs}?~<wÁãÓº?‰O%ÒÙs}?ï\†ZÄé÷?‡CU6µ–?"o4£ó%+?‡CU6µ–AGN4FGL J1427.4-1823?îã\)€@Co`|A™þÀ:_'‰±ÅÀ<YðHÒש@ l)lŠî?ý&ÆÞOâ?Âɋ9Y'î?·õºgš?öVuÂú»ó@žé€â"‰¿Òº|þƒS1¿ì¿"zM£ø?«p=]a7±¿ävH@áqŸ¿ºÝå_&s¿è1D±	ø§AGNbcuNVSS J142726-182303?ïüV]ç?0Ç''÷ã?=M°–Ú?0Ç''÷ã?ïîáa_?wäBP"Â?a€šbw?wäBP"Â?ïïÿ($ó?Z'5¢óæ9?`óñøv?Z'5¢óæ9?ïöi(bŸ²?=ŒQ4Ð?S-¯Ä[i?=ŒQ4Ð?ïö á•x?Gú0mÞc?R¾<¿åè?Gú0mÞc?ïÀ>¢/ÈÎ?…þâfª?à®Éß	?…þâfª?ïí	7ƒœO?oËÿxۆ?böÈy¤b?oËÿxۆ?ï׆{Ñÿß?gñ' ?t<Âo¬†?gñ' AGN4FGL J1427.6-3305?˜¢«4MnÜ@9–r§½HËÀ8ŇB_ À;Ȓ%1ñ@B†Òeh@–'³ÌJÇ?¥C8cõ?¾"yNõ†@¡aä÷f@SÅm2¿Õ©ma­D¿Ö¹ã»üšñ¿äe0Áhë|¿ærᏥ¿ål¦â,…o¿æ\_©÷AGNbll3FGL J1427.6-3305PKS 1424-328?ïû³×™–??YájîR?C©/æ®êt??YájîR?ïâü;Ð:À?"…îßȓ?mÄ	IŸÅ?"…îßȓ?ïÆÏ:mí¢?
ǃà"_?|˜b¿jG?
ǃà"_?ïüÇü$ö|?&ðĪF?9À_YáW?&ðĪF?ï÷ãýHž2?PÁ‹ú?cÓ?P8(«"G?PÁ‹ú?cÓ?ï‡÷žî©R?ÑB€Z˜?ŽGÅG?ÑB€Z˜?ïÀ6ò"º?…hÒC²›ï?ä†ï÷2ø?…hÒC²›ï?ïðÏÙF­¹?P';<PB*?^`Mñ,Ž?P';<PB*AGN4FGL J1427.7-3215?ÚªãU¯@:X_9K{)À:-70îµUÀ<C¯æâøˆ@¢Éübç@ѽaõ¾^?¹ô%j‰?pGڊ$±?·­=+H@å?›\'?ɛj^˜'¿èO¯'Âe¿âPmk=e¼¿âT§BÔ¿ãÌ'áE¼¿ÈÚ*~…AGNbll3FGL J1427.8-3215NVSS J142750-321515?ïþCÎû"û?}x'??+Ã
TlyK?}x'??ïôW&œ:Í?ZbB+ÔÞ?WQ²\V•ª?ZbB+ÔÞ?ïù_mßèš?7m­NH?J'HCW½'?7m­NH?ïÿD©Û¹­?+j¸.úÔ?jÌÝg5¨?+j¸.úÔ?ïýðr].s?&7ƒN<?0|m#¾+?&7ƒN<?ïÏp],£D?Qþ$ˆ x?xGÑzÜj$?Qþ$ˆ x?ïû'·Ï©?Mo]ƒË¸Ô?A·ýgÀq?Mo]ƒË¸Ô?ïþÐx[?.xt…zM?(ù£%N»?.xt…zMAGN4FGL J1427.9-4206?á š(4Ò@1DûC؜åÀ5µ¥BDH.À:'¨æ=·@áÃ;Ôl~@Å,?#+~?}P>à$=X?¶­ÿ7¿E@1tÿ†]}@#ÐÜÑқ¿Áã¸á2Š¿ÝÍ+—]7¿ã¢U_­å¿âÿÀ?Ѐ¿ç¡¢4¿¿ê¤0+@öjAGNFSRQ3FGL J1427.9-4206PKS 1424-41?ïäQ¦ïK0?h·)0R¾¡?k®Ys@f?h·)0R¾¡?æUë°42?ÒPNí#?ÓTÄ(Ÿ—œ?ÒPNí#?íž^Jye?¦òÃíU\?³
gÑöW?¦òÃíU\?ïvfB=x?¥6¥ ¾ïó?'3=w¸Pò?¥6¥ ¾ïó?ïÖS¡ñ4"?v
|?G'Û?tÖ/Sr?v
|?G'Û?ÕHÖÌD?Õg0زU ?å[üx"™Þ?Õg0زU ?ïk[]žÁ¢?"(52¤³w?'""QO5Å?"(52¤³w?èáa%×"?È•Ãîy<?Îz{h£z?È•Ãîy<MIXED4FGL J1428.1+1629?ïö³_µ¿Œ@PMØ/×^ À:EçjÝÄÀ<UŠ"C"@ŽZ"Zî
@‡ëy`>.?½?s³VB?½ËÓþo\.?ûöÚ7›@§EaE•?îäӉp#¿æ2-¿€Þã¿å¾Tdc¿êß !s¿ê}'gv0ß¿ðAGNbcu3FGL J1427.2+1610MG1 J142813+1629?ïøöS;?KCÅlFuŒ?L'¸´œ"H?KCÅlFuŒ?ïè™FÒ;?rìÀb§.I?gÿfšñ4ï?rìÀb§.I?ïÌ%/íáù?yߏqËgÿ?yígøã¦?yߏqËgÿ?ï[$ë`¥v?~@Ùx§'ž?"›bŽÃçF?~@Ùx§'ž?ïì+»€ÛC?c€·~HD?cÔDˆÃ¥?c€·~HD?ï~ÜÊë¿?˜ïíÕL?$fÀ$&?˜ïíÕL?籠"')?‡Ü&€'Æ?†žÞԖ'©?‡Ü&€'Æ?ì¤-ÐY?£ÆgÛjü!?ºÞ'}7ۆ?£ÆgÛjü!AGN4FGL J1428.3+5635?Ïo—§üÞ¸@Këæ`ɊÀ;rrä#+À<€ß×@ϔ*ÄϨ@Mv«Xÿ?Ñj;<ìðY?ÃãC]©~?ò†	êdH@Pÿߞ¶¿ë¦ %9um¿Î›C踿ålZÁ'œ¿æ£ßÙj¿ïÿb%>Ô?ètÛߏG0AGNfsrq87GB 142651.1+564919?ïþO¡ªŠ?%PAQ}!ô?+¢ìz®!?%PAQ}!ô?ïö1¤V¥Ã?TrcþŒÍU?Sœ·ºº‰?TrcþŒÍU?ïÎ\˜B'³?p‹
!!|?xѳ؇Z›?p‹
!!|?ïöÆ̾Æ5?>›swyKg?Rrfí§eC?>›swyKg?ïþƒÇ±k.?,±­ëÂҔ?'ÄJø¿[?,±­ëÂҔ?ïÖ{t
Í?vi'Ís
?tÂEþȍš?vi'Ís
?ÎBÕ?…ør'Ëç?ŠX' vÛ?…ør'Ëç?ï¿Wtû?qªßc¾›{?€:j0¶±K?qªßc¾›{AGN4FGL J1428.5+4240¿àOšSöÃ@P9©¨–hÀ9t"à4êÀ;ÿO†Pº@!¥ÿƒƒX?ù°³â;ë?«6ý[ú–x?•'ßÿë™R?í?jCj¸Û@f;¥¿é1•Ùñx~?èR€f­¿Óù
'åÍû¿ÙL;l茿ÊÓ¤—Ïj¿Êß"$m¹AGNbll3FGL J1428.5+4240H 1426+428?ïþ"b£
a?gÈÏA)c?&¹Ñèάâ?gÈÏA)c?ïöuUþ k?Wü·"ж?SSكÚå?Wü·"ж?ïí;±ÿ8|?p'b|i5?bÄN'C#‹?p'b|i5?ïëèxú½¡?QÖxL¸Úm?d†ö$5?QÖxL¸Úm?ïü´WFI!?3î_ÀçRä?:]Fûæa?3î_ÀçRä?ïÙ_{ÕRF?z}Ôé'0?sPB/säÀ?z}Ôé'0?ïæŠÝ'ìH?wŒ»æNÁÃ?iu"±MÇá?wŒ»æNÁÃ?ïÙ"Ù&€?fßg% p?sqn¡Ûï?fßg% pAGN4FGL J1428.7-1017?堄gáÄ3@Fà:S¸ä¸À;I|­ÐˆCÀ<œFÙÙ$Ê@#
‡þZä?öõbÓ3ï?ӗ…"P??ÑI¬|]I?úèââ¸Ç\@þÁFÆ8¿ïÿT_™?ÝN=»!~«?6Ã
¬?ÜZ'±m˵¿àn¹ª?¾ëƞE·AGNbcu1RXS J142844.4-101801?ïü&ɏÍà?3r|Û$L?>ɱ`5g_?3r|Û$L?ïã(%?añ‰Ài¯J?a`HSњY?añ‰Ài¯J?ïÐÜ4"þ?v{
Å?w'åË?fÅ?v{
Å?ïêÝ'86?Vôi^U-?e"Ø°Mj¸?Vôi^U-?ïû±aanÛ?9{ëù'ÌD?A:{{¹±?9{ëù'ÌD?ï·'ªz#?ˆƒ=Û¯s?'9¶]?ˆƒ=Û¯s?ïÝapÄt?xLÝþ)?qqÏD.)Ê?xLÝþ)?ïÏ:µ³?rÑfŒÁaç?xb±DÂçñ?rÑfŒÁaçAGN4FGL J1428.8+7429?Áº²ðúöÎ@D'À~áÀ;s֑q­À<ÿž)\ñ@!}@¢‡~å?þË׿o8?½Ӑ¶¿¶s"ölƒa?ú{x| @	#pš…?ïâ½—¥¤¿¨nâXFµ¿æwÂ,ém¿â°â`‡Õ¿âd ()ö?"cþ	äAGNbcuRX J1428.4+7429?ïÿS"ù?àï1Õ?€ÎÃÞû?àï1Õ?ïõÕ·#Ÿ?V®¸dµâ%?TT'—²p?V®¸dµâ%?ïô|¾x?aå©#çœ?W",ÂR?aå©#çœ?ï÷lÜŽ?<N>y ?Qç&šg'˜?<N>y ?ïÿ…yjê?99¯Ue?ïMM	Kð?99¯Ue?ïÛóê%«¿?r9G&^©N?rf°w?r9G&^©N?ïñ_Uro¬?lÛtMã@?]ATºë™"?lÛtMã@?ïÐ8¤â"?mJÄ…P"?w㭅PÆ?mJÄ…P"AGN4FGL J1428.9+5406¿Ï¾mt³ÂK@LÑM"‰aÀ:¾VCæÀ<Ÿñpv‹@ЉÒ|97@èÃm¨z?Ço<8j¦?¿ƒb¯È°?ôOÆl`{@¶¥ÇzS¿Î~¨<¿3¿êm-]0]¿âP÷†®¿ì¹›Aº_¿ÝäYüu±Þ¿ïÿ-r)HAGNfsrqS4 1427+543?ïþ¼ÜÈK?HcÅξ?$23Œæ'®?HcÅξ?ï÷Ø>ùn?S‹KüÄh{?QòP½Ô
?S‹KüÄh{?ïÌ' ?ƒl®"îdž?yóñî‰#ï?ƒl®"îdž?ïû$õ
Œ)?-ƒïÓRóü?Cl+—#J¢?-ƒïÓRóü?ïýã¿úÏ?5¶na‹Ç?7ˆáÿ¿?5¶na‹Ç?ïÝÆõX˜?tD-\??q}œ~t{Ý?tD-\??ïώñÓu?']'Þ4a?x8‡·"?']'Þ4a?ïåVkœ†3?[uÎa¾?j©"šsŒ©?[uÎa¾AGN4FGL J1429.8-3058?ï͍eiøR@;Voç¨mÀ;&Ìÿ!³¯À<'ütðm@ ´1ð'ú™?ÿ¬ÇÔ?ˆ?ÌZ.õ‹ÝÄ?ªŸFàAÒ;?äþraFl?þ(V†?u?ï]}>o&~?ìl]¡Eà_¿èç£è§ô¦¿ØUÃ`½Z¿ì¦€‡ÏÃ?ßOµIùHVAGNbcuNVSS J142940-310013?ïú:è£î?DÎBZiY?G^I6n,?DÎBZiY?ïÏ
PÂ݂?…ŒôÇCŸ?xyW°o6Ø?…ŒôÇCŸ?ﳫ,C?|±«c–?ƒ?qÍÕ8?|±«c–?ïŕ¡ùu³?fòˆòM'
?}5/´ÂB?fòˆòM'
?ïúãy?9¯?HîDÂ!"]?Dr<£ë?HîDÂ!"]?ïVk*E?¢šä·?•<œš·Q?¢šä·?ïÇL7ïŽ ?©×5x¶4?|Yä—‡¶?©×5x¶4?î´XNöˆ2?"¸Ahe?¤º{Çâ?"¸AheAGN4FGL J1431.1-3120?ïÿ6tŽÐÆ@:ßlœ
"À9ÛÖ¶Zš€À</OC427@òˆQ¬y?þ̦6`^?¹"y™I?³¼f"HÕ1?ûº"ԗœ@-îdÍ	?ïÇ P ¿æçÌÍ£Œb¿ÑíÔñhŽ¿àŸß|&í¿Ý¡l å}É¿Üå6%+ÁAGNbllPKS 1428-311?ïÿ"›>F?[¡Lï?m)Yþå?[¡Lï?ïò¦\fÕ?mzˆX'áï?Z³GîF°?mzˆX'áï?ïöìɉÚ?Töd2–?R&nNž:ì?Töd2–?ïÿ
BÍsÕ?
õnB«Š?W N4X‡?
õnB«Š?ïÿÌgnœ?¸07>?Fo
ú‹?¸07>?ïÍAŸù8?#ŒTÀ)Y?y_8µÐ<?#ŒTÀ)Y?ïôÙÇÃ3Ø?cç×?VLp¶o¢?cç×?ïþx–i¹W?‹|Rü?(v—ÄÍ2?‹|RüAGN4FGL J1432.2+5051¿ï`Ù²õqm@MÄ}¡ìNrÀ;Œ¡c'wÀ<ÓGºÇè@âõLÈ°ˆ@Ú6º§0[?Á³±]Z¤?Šo*%sÇ?ÈÔÁÔiy@
qŽ¯/Øá¿ëÿ˒:)Ç¿ßii:¬#_¿å÷·ÒiſݑÅÚ뛿é"±œ]™¿×œªZ±ý>AGNbcuNVSS J143217+505603?ïþ†Œ\ÖV?HyòO­?'—:μ?HyòO­?ï÷º''ô?QÆKÍ®?P‹Æ«ù(-?QÆKÍ®?ïð]ÕçB?YƒMÅ`<ñ?_Eø:=]?YƒMÅ`<ñ?ïýG6}óÿ? ÛׅDfœ?5ÆJ6|N®? ÛׅDfœ?ïû•ŠkS`?;·ŠH:s?A©Öw‡èÕ?;·ŠH:s?ïÛGxSg ?vÕmêÝ?r\CËMp?vÕmêÝ?ïçü?În…?r?|©h)?hÀV+T?r?|©h)?ïö¨óÿ–¤?C'ÊC~k8?R®ÝÈü?C'ÊC~k8AGN4FGL J1432.8+7648¿ëÏu!{a@Co8q`•lÀ:ôÞü*ˆÀ<Äh-ƒ@
Ž+§M·@Œð=ë?ÀA°¹ñ¨Ï¿±¸©)Y•ž?ðôu£KÜ?øS¸8ìË?Òpõ5¡¢}¿ä‡£'¦ô¿åJù"–,þ¿æ°ÔéÑÀR¿ÍÇNH7|C¿ïûܟ¨§TAGNbcuGALEXASC J143211.35+764355.6?ïû–jK^‰?7ªà…eT?A¦W±,‰Q?7ªà…eT?ï݆]I(µ?tÓÂÝz7?q<ÑJí…p?tÓÂÝz7?ïÜB}ðÌ?nmG»ßI?qÞÁzùé?nmG»ßI?ïŀiê è?c§Í)åâ?}?Êôò"?c§Í)åâ?ïð`xÜ?XÖ(^w"?_?'ÒtV?XÖ(^w"?îç6LS|?§²òÕ ã?¡Üžªd=?§²òÕ ã?ïÏÓZ/?|A%¹?xqF—P®?|A%¹?í‡Äøm¡?£èz õœ?³ÁØ=sqõ?£èz õœAGN4FGL J1433.0-1801?ÊTU¤™ŸE@CIM½øôsÀ::DZ°èÀ<~ó%&*@u2¹e¼È@(ãúü?ÂÆñÁxÛ´?Õ}BuñI@	'^VÍl/@ù
ÒÁÙ?×Ýê¬\¿Ó(ؼD>s¿éS³`À	E¿êR·ÈXÉÆ¿èÕÙ ð¥ð¿ïÿì»"AGNfsrqPKS 1430-178?ïÜçGUË?rr4#íËÃ?qŒ\Xì6g?rr4#íËÃ?ïòHGþ'Ž?_û¡9Ñ.?[ooê=´ã?_û¡9Ñ.?îŽ9'"Ñ?™BMõ"»Œ?§fÖd÷?™BMõ"»Œ?ïüÝ{›¬Ä?#øଵ?9!ì‰ì]?#øଵ?ïϵ?<€å?zK3aV´#?x%`ce?zK3aV´#?ïº
ó2½?"Ҟv?|ƒCîB?"Ҟv?ím®¤÷#k?£5®à*É?´'ŠØ´Ø'?£5®à*É?ïñv>9^?Nðua…U?]ƒy¡s"?Nðua…UAGN4FGL J1433.7-7304¿è*1Q†°^À'`†`ÔÀ;°¥R4€:À<Ï0é¬×@#1©kž´Œ?ڐþ?‹†1?ãќ	¶b'?ïù½€Ô{Ã@®ì?þÛ3,}6?ëå² ùõ¥¿îޜ¾H'¿ïԋÝï4?ïŒv›gÏó¿Ç{ô'žUk¿Ï¡&Á4éAGNbcu1RXS J143343.2-730433?ïõßü2½?P¯ÓáI̟?T@TL¦S?P¯ÓáI̟?ïáÆyK›_?{àÓ`?n9†ç>ØÎ?{àÓ`?ïwwš//‡?‡4'ž¼?'³:×!?‡4'ž¼?ïô6˜N7?Q!?Òë*I?W'Å:—`›?Q!?Òë*I?ïàLnÌ&?uŸ äýsE?o³'Oc¹?uŸ äýsE?…åï?¤«x|-¡?ŒZ|o´7?¤«x|-¡?ïB®øjNA?"><8°ï£?—ª ö%ÓÓ?"><8°ï£?ï圃rª†?nšk|'Q?jc|¼)?nšk|'QAGN4FGL J1434.2+4204?îWø—€å™@PC¿rq7À:GÞ
ò}À<¡("V@éùK/ÿ@—!œ1ú?¶ÍàsØ(?‹¨Mˆì?ш¾ÀoœE@_ˆü"d¿áÀç@Áf<¿æÉì}l<i¿æS.°ís6¿ãFñ÷(Àé¿ê''ÿNTL¿ïÿÉ¿&FAGNfsrq3FGL J1434.1+4203B3 1432+422?ïúçXØøï?6fa‡ÆÃ?Dbšü×?6fa‡ÆÃ?ïõ¦0'ÿX?W×rš2ºø?T³žüý"?W×rš2ºø?ïçjè?gQºòI?h•þ÷šÀ[?gQºòI?ïí·ò†V?OÜÜȽ?bH
rÊÆå?OÜÜȽ?ïíÎanÒ=?` úRjPÄ?b1ž°Ê*¹?` úRjPÄ?ï܏½³æ?uȏ	J'?qþ8!&Ñ?uȏ	J'?ïá
OZˆ?vP•ÏFï?nò°b' K?vP•ÏFï?ï¾fŸ!?pµ?Næª?€f|M8Ûÿ?pµ?NæªAGN4FGL J1434.7+1950¿é´.Eì&@PR2LƒfQÀ8· ·›`À;¯–ú'è}@ْÔ-"8@)(v>K?£ß¾þQþ?ÁŒšBç±@´[זT@Â*­¨š>¿Å²@Äì-»¿ßÃp,¸Å¯¿äì|•|Ôg¿å1" Ü.¿è`½¨"¿ë‹q¾‰=AGNfsrq3FGL J1434.6+1951OQ 253?ï÷E̒ë*?QXXÄÚÀ?Qtfå(l'?QXXÄÚÀ?ïí,iH ´?rš‡¢õI?bӖ'ā?rš‡¢õI?ïŒÅe¥KT?U'JùJ?ŒÎ¦Íó%?U'JùJ?ïõŒÜ:î?EŒ‡2ã=Q?TæãÙ%`?EŒ‡2ã=Q?ïÝþҝ5?r0!;ª>?q–»XÃ?r0!;ª>?ïŠøòÎà?£W2nv²?AÃI	l?£W2nv²?ïR/…dê?"V@Üò'b?•¿Sb±?"V@Üò'b?ïÉ#w›S?k³Q¼6X?{nqOáQ?k³Q¼6XAGN4FGL J1434.8+6640?Ì1ùöZ†@G°K±¯:À;1ñÛzºÀ<äŸê²ð@!gŠS*Ÿf?ù~N"ÈQ=?ÄMoßáÒm?½£Ž¡)A(?ù`¿'țæ@=qá¿ï'ëk¿é,%Â!ù?ïý7cCœ7¿Îëð¾ïi…¿ÞšÜDŽû0¿Ðï¯OäCâAGNbll3FGL J1434.6+66401RXS J143442.0+664031?ïþ¸â‡Z?8u¨¡Á?$ÍJGƒ?8u¨¡Á?ïóðl ?X!ûiΓâ?XÕá/Æ?X!ûiΓâ?ïó?ê?"-?eŠîÈ­}Ü?Y€+µ¶T?eŠîÈ­}Ü?ïÜ¡•UV?Z÷,UI6Ã?qñ/:$Èó?Z÷,UI6Ã?ïþ+ŽÕÆ?#ñؾ7ç<?-OËʯÊ?#ñؾ7ç<?ïÖürh?yw¼zK«?töÌKY-?yw¼zK«?ïñ[.qNï?qº1¤pÂË?]I¢¤oâl?qº1¤pÂË?ï©0.•Y?w4c›7?…³ûňµÇ?w4c›7AGN4FGL J1435.3+7120?в
õ6Ã@E¼®§GØÀ<*¡/"À=˜w:Ê@:ë&ÿô?ÿ ´%6n?Ö¬æ0x?æH"Lx~—@~*šÞ=8@:¾÷!4¿ïÿúÁҝÇ?ð¿×V'þõ¾Þ¿á(ۋ¬q
¿ïþš9҉¥¿¡NöºKAGNbcuNVSS J143518+711818?í½']BÙÍ?ûÙ¶®í?²mŸW?ûÙ¶®í?ï\ù³¾<?£kÖòþUT?Ÿ4`Àñ2™?£kÖòþUT?ë›~²HÎ?®u±ÅR?í'6ÜÇ?®u±ÅR?íÑá!~¼?'6÷ûßï?±wØõ<<"?'6÷ûßï?îSÎG‡d?¸ؚgH?ªÏãóÔ¿?¸ؚgH?è™Äb)ã?ÍhCؔM¢?͘ï²wXt?ÍhCؔM¢?ç3	›po?¸íQ¦?љìÉ à?¸íQ¦?åEwÓ÷
"?¹5W›Íom?ÕuXäÚ?¹5W›ÍomAGN4FGL J1435.5+2021¿è̽öù¤¥@PRžì¿±[À:"F}'ÒÖÀ<]	ÆR_@!S«Èp?ÿ0L齞\?Ìã^ÊÙ?Ïqßy¹Õ@hÞ£Žåá@—Ò- ¿ï]ÔA5Tv?ïݤ@;¯Y¿æV>@¢Â¿ÈðšÝ;"æ¿è;`gÊ¿ðAGNbll3FGL J1435.2+2023TXS 1433+205?ïʤPNC|?{¤t^a¸>?z­×ÆP]ó?{¤t^a¸>?îñaÿEè9?«âÆ·p˜? éà	é®r?«âÆ·p˜?ï@¨Öð´€?.¦AÙÐR?—êå
8?.¦AÙÐR?í'u€?–´|ñX¢w?³ïX'6€?–´|ñX¢w?ï»B
çe?™èÈ)D´õ?žˆ—ÃÊ}d?™èÈ)D´õ?벎$Æ]ó?ƾ*ü
°'?Á5Çlæˆ5?ƾ*ü
°'?댚äX•Ô?­|ê(-¢?Á͔n¨®?­|ê(-¢?äÖ}Ü_øõ?¿qTË´I?ÖSG@?¿qTË´IAGN4FGL J1435.7+6148¿ïËÔužÎÉ@I›ÝÁç–}À;Ÿ{DDÀ<ì'ódK@ÌšY²ú@t` Ò?Ç;XE¼LÍ¿«F&CÐS.?âå7ýO@ª)¤"…?ïéóïP…T¿æxcôœ¯¿éwÙ.Úß¿·ÅC–'¹¿ã}:ÞxEâ¿ïê¶øO1–AGNbcu2MASS J14363365+6149514?ïûüU%¡O?4/´4³Ê?@«äŸõr?4/´4³Ê?ïôÀ@øBÇ?XBq¾Ûß?V}¿ÃÏ?XBq¾Ûß?ïßÕ¯Ëþ?taG$Р?p(6hé?taG$Р?ïõ§¯°?>º7ÍÅÙ?T°àL¤P?>º7ÍÅÙ?ïóíû,?Vˆyå·èÚ?XÄ%v¨?Vˆyå·èÚ?ïÕnd•3Œ?us.΅Ì?uHÍ°–Æ	?us.΅Ì?ïÏ2íŠ~ì?{¸ù	,€½?xf‰ó–2?{¸ù	,€½?ïºü8ÜPµ?rñR¹¸T?@ñÁ´¤è?rñR¹¸TAGN4FGL J1435.9-8348¿Ûƒó]7òÀ5ˆx·¡Â]À9ñ¸'ƒ$ãÀ</R1%;ú@™]f¤S@ë=Ñææ?¼ÄŸ½Ü*I?¶ª›I?øSëõ‡:@,'y@³¤¿Ö.á_+¿æÁIÁ•?¿è½0w—¿âÎý'¿ïö6¾.®¿ïüɟpÉAGNbcuPMN J1433-8340?ïü¡­™Š?.#L¯j?:ò˜>Ã?.#L¯j?ïô›™Š;i?\±M˜vÈK?VÈÍÍå?\±M˜vÈK?ïâóµnâ6?p8Êîn'½?mJ¶9'â?p8Êîn'½?ïýAì€é—?$¬qŽëÇ5?5ðœóc"Î?$¬qŽëÇ5?ïý}ºsŒr?1Ú¦*QÝJ?4,¹_z?1Ú¦*QÝJ?ïÑ°'êCš?–ϸà<Þ[?w'ëôà³#?–ϸà<Þ[?ïâÔPyÀ
?té¿V)?m+¯[¤ÍÊ?té¿V)?ïõÒãœG?FÒ*YmÎ?T[ÒLA©?FÒ*YmÎAGN4FGL J1436.9+2321¿—ßcqLE@Py©?)
»À:y|ßýÀ<Q'N"¢Â@ý1Äs7@‰
5
(?¾)j1¢ˆ?¯ç¸Ëôœ?ëSÛIgR@Ño‹þüJ¿æCŸu¦ ¿ãdc1Ù¿ä}P·
H¿é›K_ú¼t¿Ý'ù\wпïîÊM–ŒAGNfsrq3FGL J1436.8+2322PKS B1434+235?ïüÁfè?Wká¸\Ì`?9ôÉ?ð˜>?Wká¸\Ì`?ïõHÀ'?^væñmk?UÍn>þ÷?^væñmk?ïêz»:±µ?dzôx¯·?e…DºOŠÂ?dzôx¯·?ïê÷ïÛ"?Q"¥)œ¾?eòï(Õ?Q"¥)œ¾?ïöüC»t=?NKz—§^â?Rx&…Ó?NKz—§^â?ïÔiÇ¢t?~ÈàœËòÄ?uËBÇ<?~ÈàœËòÄ?ïÒUöŠ>?y *hš"a?vÕÕ­ì?y *hš"a?ï—
óõ?yíŸg#N³?Š:}?Ëæ×?yíŸg#N³AGN4FGL J1436.9+5638¿î.öF²…¾@KuâlvÀ9½Ö»cýÀ<\u¼D¿M@†òÍ<‰H?þ©GŒ†Œ?®¶cC‹	?è'u¹?ã#×?íUÙ@	äùÄQ©?íö–•[$¿äEmþ
\z¿ß1uBø";¿Ú›[慱¿Þöú2`¥\¿ÕVÄ-ÁÚAGNbll3FGL J1436.8+5639RBS 1409?ïþàbÖ¹á?òq#?!ùÑ)?òq#?ï÷!Þ«û?S#{IÀE?Q½Ìn£	Ò?S#{IÀE?ïùY|aê?RœÏ«&š?Jšs"¡›?RœÏ«&š?ïõÇÚl?A4]:ÿÁ}?TpKoO¦)?A4]:ÿÁ}?ïþgÿ:)¿?û³Î?)€(ER?û³Î?ïáþ'A·?qڕ=6"?nü+ÅÉØ?qڕ=6"?ïúöïò'?LéÔ<e?D$A=wŸ?LéÔ<e?ïï´/"dž?NRºA³+½?`KÐ-Âjz?NRºA³+½AGN4FGL J1438.0-3128?ÂW=ØÂh4@:!¦'¶(FÀ:Á"‰cÀ<[¾¤ž@Ö'-ŒÚ@9ö›Ó/½?ЁôRLÔ?֖ê<Ê5Ä@våÚºÌ@	µŽª}AŸ?ﯭ7OË¿Ùùð'Íó¿ç"ré+¨¿æfS¼?¶Ï¿ïç'JïŽ4ÁRÆ!AGNfsrqPKS 1435-311?ïÕSžã…v?¡<#=ª'?uV0¢+é?¡<#=ª'?ïåߥ9v?s+äâN³|?j ZÍÝÂ3?s+äâN³|?ïxWU¸t?'€~˜žáD?õG8C€?'€~˜žáD?ïÕúï–?X÷GüLa?u"qÆI,?X÷GüLa?ïö=ë·¸W?Oø#ðVeÙ?S"(Ü!Õ?Oø#ðVeÙ?ï§þâ§2<?`ÊC{Aú?†Gga|á?`ÊC{Aú?ï"o}?'§2ÏÚ%?œ›¼Ž°W?'§2ÏÚ%?ï.nր€?ƒ£òþ¯±Ö?š2%'h
?ƒ£òþ¯±ÖAGN4FGL J1438.5-4207¿îÝ|a>M1@0w>Õ'åÀ;g˜ûÀ<'œ£9UŒ@ ÷Öå¼]?þYÖÖ;
˜?Í0!ÌX‰?²Êö†M?äâ6kw@z7y>s?îØàkæ(¿ín¯½µƒ¿È¡šïÚîοÝÓÙ{±Ò ¿ãÉ?2Ȫ¿Ø;vBýU¬AGNbcu3FGL J1438.6-4209SUMSS J143836-420705?ïþD•ŽH?ƐæÌ6'?+¶¯‹2ð±?ƐæÌ6'?ïáIMž:à?t…ïÁäÿX?n¶²!,wç?t…ïÁäÿX?ïô«+Îv+?Dÿéa?V©¨UU9F?Dÿéa?ïêÕØ[™?H@Œ t?eð)ÿÈï"?H@Œ t?ïþ"7&=?1#Ûðã?&¼'&qvG?1#Ûðã?ïW¶ÿáD?¤õÄÉ»MÞ?•	?ƒss‡?¤õÄÉ»MÞ?ï÷ŠÜΈË?]O£=öc?PêFì^É ?]O£=öc?𢡄›²è9?q¸üB~¨C?…Ù÷Ï?q¸üB~¨CAGN4FGL J1438.6+1205?á"
rZ÷"@N\UÀü´òÀ;jœ×;»˜À<Âk"ÿ@ XÙéëÁ…?ÿª¼¡Ü^:?Ðj"2¯Ö?¤PŸªª¸ü?Õî$5inY@@šÒª?ëæoÖQ°Í¿ãg¾Šêª-¿åØl¨ŸÆÚ¿ÝÊ2ÿÚ
¿âëî›S­ý¿Ë¶^Ì>1"AGNbllRX J1438.3+1204?ïûMtŽ-'?>d€Óv²
?BÊ-ʖ)?>d€Óv²
?ïð!{®TÅ?iX?}2¡Ž?_½¥ÆW?iX?}2¡Ž?ïÀ'›áƒ¤?ƒéX~V›?ì2
.iÝ?ƒéX~V›?ïÚ}v<6+?VlÀfBÅD?rÁDÍ÷.Ÿ?VlÀfBÅD?ïü"YFv?9e<RüÃÆ??3]}Ø?9e<RüÃÆ?ïŽNW¯qü?—ì?ñë<?Œlje*?—ì?ñë<?ï΄•P‰°?¾5dûª?x½µEÝ/ø?¾5dûª?ïC¿äBE†?"ú!®Kcs?—ˆtG³D?"ú!®KcsAGN4FGL J1438.9+3710?æγS¡_-@PO6&,ºÀ9+Š¿â¿À<3"l;'@λ³tâ@zŠûq%?§0¹[Uç?»¨w­áz.@q|å-ì¢@AÇn.? ©r]H81¿á¤¢š¿æNS™Û¿ä¿-½R†`¿ëö{A"ÊÓ¿ïÿþˆ0»ŠAGNfsrq3FGL J1438.7+3710B2 1436+37B?ïõòˆH8~?K‰0ç…å?Tï´G3µ?K‰0ç…å?ïô	ÝNz6?^&Á[xK?WìEs‰²ï?^&Á[xK?ﲡ#6÷õ?~¢]Á³à^?ƒW·:µ?~¢]Á³à^?ïû罜‹Å?,èŽ@˜‹?@a	C™\†?,èŽ@˜‹?ïô· ÑØa?PžêoT¶Ž?V¾±…Žj?PžêoT¶Ž?ïÔkê+NÛ?"®Ö+k?uÊ
Òû:Í?"®Ö+k?ïõÅÛR2?ƒ›Éήaò?~%#"ò÷?ƒ›Éήaò?ïôÄeÓ¢?GÂzJ^G?Vw4H=Ò»?GÂzJ^GAGN4FGL J1439.3+3932?î°7…äl@PêÈ`V'À9åßÁœ"À<cv­‡@ú—Ý+ê•?ÿ<ÛØÙJŠ?±ÍFšC7¸?"'¬¨{E?áªSÆP±É@¸ï&&?ï"ÞnµÀ¿àç­=»Lr¿Û×!ºdë¿áKs›Ù¿Ú|[Wð¿å§«ÅìAGNbll3FGL J1439.2+3931PG 1437+398?ïþiö`;? l|pš?.‰^"6? l|pš?ïöן 9?V(" ¼4?RQÒêúÞy?V(" ¼4?ïöÂLWU?V~x¶|`?R{hSÂõ?V~x¶|`?ïëó«UP6?N7"-·³?dT¥0j?N7"-·³?ïûÛ
R>f?5u¡é©²{?@"ת'?5u¡é©²{?ï܉bÐì?w¥…
ða»?qý»_ŕÿ?w¥…
ða»?ïï7ҙ`?q¢¶è É?`È-`g"?q¢¶è É?ïÙ³4AÈo?`ë¬ûçè•?s&eǾpÃ?`ë¬ûçè•AGN4FGL J1439.5-2525?Ë#•Ñü­@?ZäâmHÀ;VìÔªÀ<"1í¸ÕŸ@!¡[YíÝ?ùˆ²¡)±?Ð<`CÃX?ÊH)åV±h?ü‰l«$™?÷˜ùöüv3?áÕT%B|?ït§!A™(?Ìóä餿Í=þhPK¿ÖagäjÎ*¿ã9oÀtzAGNbcuNVSS J143934-252458?ïø"¦sÖ?KTªÀYǺ?Ouf
â0?KTªÀYǺ?ï|™	7ˆ?˜üâ!k'?lÞá³tó?˜üâ!k'?ïÂ5Ô(‹?{S<ÙËF?~åø¦k?{S<ÙËF?ïQMaKŽ8?|~Ǜ‰'¦?•ÖSӝ?|~Ǜ‰'¦?ïñ6\™š,?YҍڵIú?]"FþFy?YҍڵIú?î5¹3׌³?¸Lw?ç?¬¤lÃcÍ?¸Lw?ç?ïš}ðÚ¢?ŠÐ=Ñ?‰`ƒòj–?ŠÐ=Ñ?í¹NÀ#éa?ŸñwHƒHí?²5‰þÍü?ŸñwHƒHíAGN4FGL J1439.7+4958?ïÇÅàä¾@M–ýuâlÀ9±vi騦À<~[òoÅ@ó@7'´z@0«~žk?¯ey"øõÂ?¦&ŒÝ9¬?öa	ÐcZB@¨öæ%ä?ïôÁrüvß¿ã±b]Ã)¶¿åªbÆ[¿åÕò—Ÿï¿ÝnÊ£|ÇQ¿ïÿ–]ÏéãAGNbll3FGL J1440.1+4955GB6 J1439+4958?ïî½{²94?ŸÄ P}?aB"
\l?ŸÄ P}?ïö»>–#ÿ?UKmç7$æ?R‰'~±?UKmç7$æ?ïñ"G½PO?cðæÏÕz?\Ùp^ãÁU?cðæÏÕz?ïõ·>g'+?@Z¹ôl58?T'ƒ¯OHö?@Z¹ôl58?ïû#Ðæô?Gq+È¥»?Cs ÿ%ì?Gq+È¥»?ïÛIº^?uQÚOÛ¢5?r~ù½–-?uQÚOÛ¢5?ïé\o…¡?péf°±É?f£ §?péf°±É?ïçÛ6?VÛ¶MÈ…?h$å+'(©?VÛ¶MÈ…AGN4FGL J1439.9-3953¿áýƒø·P(@2_ûz_A¯À:WKtr˜¤À<Eˆt®'Æ@ ¯ÔH@ïÏÃøõ?ºB3@Êž¿ ±ÇÈªÿ?箨—›@ûÐE}8?ïþ*"y¿¼WÆåW¿éiæM§RÀ¿ÓýãÆ
–¿áWpßçÞ¿Ü -1'r"AGNbll3FGL J1440.0-39551RXS J143949.8-395524?ïý…—./h?)‹Éê	,?3ÓDiܺ(?)‹Éê	,?ïë5f¥aµ?r.Xu:~Q?dʙ.£K0?r.Xu:~Q?ïï}Æِ?eÍN§?`'o i@?eÍN§?ïù¢¥Îk?0JŸ4?IulGÉKT?0JŸ4?ïùŠÏ–¡?G£à­œáC?IÔÁò]Ǻ?G£à­œáC?ï‹<øÀó?š)KË&ü»?0ÁÓo_Q?š)KË&ü»?ïë
ª±?qxÖ'á?dæ€ë¶f–?qxÖ'á?ïç›jT1°?Tíøz"?hd•Ÿo·•?Tíøz"AGN4FGL J1440.0-2343?îµP <²@@elaR*oÀ:!…óÊg˜À<OþR€ÖT@vq·þ4@†ý»'"?¶÷*nh"g¿œ[¶ùÀ–?å®:ÀÆ.M@´t'ˆÛÜ?ïõi~sÎY¿éF
¹üæ¿á?ž¡cê¿ÙBÔ{lÝÏ¿ä¯ÄH™ÌÅ¿š"!J'–AGNbllPMN J1439-2341?ïýٔÜE'?%$zÄö™?13W6¾h?%$zÄö™?ïòO'ÛfC?e>ŠŽ‰?[a¯óý+"?e>ŠŽ‰?ïö-6øm?dËhÈè#?SÙ¥?˜…î?dËhÈè#?ïùð›LæÒ?2!®ÀŠÂ?H=')®?2!®ÀŠÂ?ïýפ?3½Ë‡šß?7G6¥eé?3½Ë‡šß?ïǨ¢Ã[V?€ûëõ?J?|+®†ôüñ?€ûëõ?J?ïïC#›+?w@$õ6/2?`¼Ü`†Ý
?w@$õ6/2?ïî
Í{¦ó?P±!+cý÷?aò2c\Í2?P±!+cý÷AGN4FGL J1440.0-1530?Ĩ!&–AË@CïìÃã?À9"卍óÀ;ß>>)0{@œ%"¤DÃ@½´'l¤?µ ªDŒ¡ä?–è>€¡Ú?ä&áìÂ@@beOåñ?ïöÒYԇ¬¿ä³5è³2¿åŽF´ð75¿ãkã]²ã˜¿Ýg5c'¿åò#žj¹²AGNbll3FGL J1440.2-1538PKS 1437-153?ïþ6ž‹?  }'C?,–^QùÇ?  }'C?ïôÁ'ìs?YDðí4î—?V|ۖëÉ¥?YDðí4î—?ïëI*§"¥?p6y]<ݳ?d¶Õ€VÒÍ?p6y]<ݳ?ïÿ\Eóv§?ÉÞRRª"?wHþq£æ?ÉÞRRª"?ïý#œè.?2'%>I4Ü?7&â1ØÔ?2'%>I4Ü?ï͉Ž<L?µ~{Øö?yx»dú2?µ~{Øö?ïފ'ž0`?{"hÄâ`?pº¶•jð@?{"hÄâ`?ïþ˒îD?v¡"ÐV"?#FÎêb¨?v¡"ÐV"AGN4FGL J1440.6-3846?£Û
ãZ'O@3S™åóíÀ9›Ò<xVSÀ;ýF[.$@!ˆjüx6?úËP`j£ã?¶>iN?S?¨H‡-[X?óÏ
D& ~@P7~òNg?ïÿîBt!¿è•Óa'¿à—«öÐ+¿Ï 	cr–¿Ö;'}E¥ü¿ÐŸ[DÊ4lAGNbll3FGL J1440.4-38451RXS J144037.4-384658?ïùú^o:å??´s!üF?H†é$???´s!üF?ïޕám­?rʤ"?pµ=Íýb?rʤ"?ï×,#õR¨?taDˆ²Ú?tiíô( !?taDˆ²Ú?ïÚÑ…6¿?]m&ŽÕ?r—x75T­?]m&ŽÕ?ï÷)†zò©?J Ó͌`	?Q¬ómlî?J Ó͌`	?ï[†K«q?¤Qœ3_¥m?"/-ó‹Ü?¤Qœ3_¥m?ï»\|O(T?"ŽÝG'ñ?(àíí¹?"ŽÝG'ñ?ï}Ê÷h4z?}{êÙVÞ?F¡بª?}{êÙVÞAGN4FGL J1440.9+0609?ã;‹úÓ@LJ@c^JÀ9¦K»À5À;ÿˆ}£–@ÆK‰Á4h@uv'[¸?¹XÙµé[y?®ê£§dˆ?ñnkÝËù@
'?úTz?í=b.$¿äõϏõ«é¿á̀v²å¿àùÊÇ9¿án"áÉ´¿ân@$ˆKAGNbll3FGL J1440.9+0610PMN J1440+0610?ïþÿwD<?µ…R÷ic? ‰ø‰Ÿ#?µ…R÷ic?ïð?›ÔåÔ?cè¥Ü£"'?_€È»9;?cè¥Ü£"'?ïñ¼@–%Ï?hæŽÉ»V?\‡~ÛóqT?hæŽÉ»V?ïô8$oÝ?BŠ±[iî?W·0Ãî2?BŠ±[iî?ïþòù©œ?"!²Ùk©j? Ðhýoë|?"!²Ùk©j?ï­íhù"ª?—>n¥¥¤?""¥·LA~?—>n¥¥¤?ïðªK‡V»?p_7/X"ƒ?^«iQ‡š?p_7/X"ƒ?ïÞ_¹E}Û?`Rbîé?pÐ#cp^€?`RbîéAGN4FGL J1441.6-1522?äi.Uº@CäU•:À:M0o3"'À;ßr)Zl@&+Í@ð¶ß$¾%?ÈUÛ~ÁQ?ÁªQ¢µ?øñzç&ë&@
¾Ûc9¿ës­ÁnË?ïýž%ðT'¿èš[@BH¿åªª˜Å^D¿àCnI‰¶Î¿ïÿÿÊPËAGNfsrq1FGL J1441.7-1538PMN J1441-1523?ïüH*f0?@jÆx
:Æ?=¾®â©Þ?@jÆx
:Æ?ïð48ñ?dŽMüÞEš?_—JP‰B?dŽMüÞEš?ïÒCàDË?x¬ô
Ý?vÞ{â6?x¬ô
Ý?ï÷FG"p_?:ï±Ã,—?Qsp½eÒF?:ï±Ã,—?ïðþqyXË?`e @ìG$?^&™p?`e @ìG$?bÝ?‹±?!¨ìÿºc?€ŸH¡®·Ë?!¨ìÿºc?ï T,ð4?˜ú‡@Èu?›õ~zaùx?˜ú‡@Èu?￵èã6y?uÿ?
`è?€…·¼#Å?uÿ?
`èAGN4FGL J1441.7+1836?ʹ4‡¤­'@O¢ Ç`À:€œߢ'À<}šYù@REP—@zŘûå?¿dqēm[?°:ŸŸíò?ëæ±Oí@žÍØ¯¿êéôæÇJ¿ÐõùìÀˆ¿Æ4A{†¿ä¾âÿ>9!¿àÙ O–@I¿ÛÅu€	ЎAGNbcuNVSS J144143+183706?ïûÏdŠKÑ?6ú'ibø?@ÂnBã?6ú'ibø?ïõnP.…h?\9ÏäÂ'{?U#_f|¸?\9ÏäÂ'{?ïäWùL©?pÁ­ä¶@?k¨®?pÁ­ä¶@?ïç¥^QwŸ?P°¬°¢Ÿ¨?hZ¡å' 7?P°¬°¢Ÿ¨?ïóc¶¢'»?Tú¢VÚ<Ú?Y8'A?Tú¢VÚ<Ú?ïÈ!ݨð­?‡]Y†àÙ?{ï/§1c?‡]Y†àÙ?ïÕÒº
e?|Ä<s6x?u£6}–?|Ä<s6x?פּË+b?p!ÅÜEv9?"žÍ1·ã%?p!ÅÜEv9AGN4FGL J1442.0+4348¿±ŽÛÓåj´@O"úÖËSÀ:x˲À<¯Ä
†k¿@J,\\×?ÿzΝ‡dä?À"¡²í©?µ2»"?÷™WÚ²h@"(¶ØnÁ?î钀J¾¿Þƒº¿Ùõ)¿â!Êö2÷¤¿Ùk*ñER¿âPŠ\ô¿ïÿÂÞ6œAGNbll3FGL J1442.0+4348SDSS J144207.15+434836.6?ïýnþG?&—.ÀyhB?3"ž"?&—.ÀyhB?ïó4O½Øh?^Žþümûæ?Y—`É_4?^Žþümûæ?ïòZï
®?c•öWMÚT?[KÈeC­?c•öWMÚT?ïÖF÷3Ü?Vñ|ÿäâý?tÜþ""YÔ?Vñ|ÿäâý?ïû3†®õ?=,¢Ý±E?C1æ{(?=,¢Ý±E?ïÔ#k}?xøæw[í?uîJ2—™?xøæw[í?ïì3f×þ?p©2ÊÊÂ?c̘勪Ú?p©2ÊÊÂ?ïŒæ¸çŠ?t<kÆ@¤]?ŒÆ\5¹y?t<kÆ@¤]AGN4FGL J1442.2+0622¿‰ãoÈwf@L>@(äüÀ:_Ê?SÒæÀ;̒Ü6¯@q§£áò@"†ŸÁÑÇ?ÆXã["‹?ÔjÛöÀf@Ž†ƒ<`@vå¿â€)«|ñ¿Ð%?•í¿è˜b'+=ñ¿æô¥žµ@¿ïÿå}ó Ì?íýݱ žÜAGNbcuSDSS J144212.23+062526.1?ïô³ó-?br-‰?V™ÒJÏTç?br-‰?ïãÞoÈ ÿ?z:ÄԈ;y?l!,`@À?z:ÄԈ;y?îl÷©p?˜ÅWÒ¨C?©>pý6ú?˜ÅWÒ¨C?ïñÎ,¯q®?N¯à~q?\c§O2³?N¯à~q?ïñۆñBÅ?eõ%gâÍ?\HòYó•$?eõ%gâÍ?ïâ‹9ì?±Už¾ÎÖ?žƒ¾pPŠ?±Už¾ÎÖ?ëýÒþ®á?§â­¹ÖÜ?À˜´D|?§â­¹ÖÜ?îø@ÂN)ë?—€,—*? {óÚAzU?—€,—*AGN4FGL J1442.6-4623¿Â;{8…ƒ@(•¶^Ì>2À:Žö¨hiÀ<-_²@ sZwÅ´U?ÿȺiú?¸`u¡æv?"¾¬Åè¤f?܏Û_Œ­x@û-+û¿åՔ«W?ïúhai¿¼…
ìB3¿Þ<ǼAº5¿ã(qGпÜk:¡±SAGNbllSUMSS J144236-462302?ïývÄÇ4?%ƒíìÖ?3"I±Ð	?%ƒíìÖ?ïåÃ>ê²¢?wæOå!€¤?j<ÀôQ?wæOå!€¤?ïòšÀúËR?f'žT»*z?ZÊ~
)Ù?f'žT»*z?ïô(˜œæÍ?DèÓ*7˜â?W®Ïiô¬?DèÓ*7˜â?ïúêÕ ƒX?;2[¤\TÔ?DT«nøÈ?;2[¤\TÔ?ïlð"?ªÀeå{ß
?R	W"?ªÀeå{ß
?ïî@ò«P?qÝr¡Zº?a¿}åy8?qÝr¡Zº?ïäØå3öÓ?_áõ»qóE?k'ü#µ8?_áõ»qóEAGN4FGL J1442.7+1200¿Ý>dÈ4?U@MëöÂiœ|À9èóɐØ*À<1<°Švç@ €&˜ðý?úÏÀÒÆÓ?¸Äßîg§.?¼'‰¡m½7@?¹£ûk@ÜíUÔ¿ï¶PÕÛi?ìyK!K¿Û±EC_¿ÁwkFud¿âï6ÀÁ&¿Ù¤4'NùbAGNbll3FGL J1442.8+12001ES 1440+122?ïýfN#à–?0‡%,·?4͍Éë"?0‡%,·?ïãXr)`?u"Ùra«?l€§‰·o?u"Ùra«?ïáޔ `ˆ?p
îoۗW?n!k;ß©?p
îoۗW?ï†oI¨¯P?rI²jƇ?Žd-‹…X?rI²jƇ?ïóg'ð¿?Z>
%&?Y0ÜDýž›?Z>
%&?ï[@k]¤©?Ÿj<3âۂ?"—ò"KjÑ?Ÿj<3âۂ?ï¾R¢‹G?".õ¬'?€kWz"èG?".õ¬'?îCŽ^
b¥?›¹8XQžÛ?«ÇMî¬?›¹8XQžÛAGN4FGL J1443.1+5201¿ê¡QFÍ!@L¾Ç¸Õ¦À;X"%"À<ä@¨f»÷@È,å'?ÿ,^YQ«?Çw*Cuu£?ÀåOe´?øÄÉþ¼3"@*0aFÁÛ¿ÆǪ5¿à\¶úS¿á䠓ˆÞ`¿ß"ãÍy¿ß™Ì$0`ñ¿ç/Ç~fAGNrdg3FGL J1442.6+51563C 303?ïý4›	©?,d•'–ñÕ?7].Ë?,d•'–ñÕ?ïíöjÕáÉ?aŪR$><?b	•E›|?aŪR$><?ïó¬þPº?Oҝa"ƒŸ?X¦ÝÔ£Ý?Oҝa"ƒŸ?ïʃ ¢¼?Yßðø>?z¾/¥²ö?Yßðø>?ïòKü¥$	?Y­ûÕ.÷?[hÿï~?Y­ûÕ.÷?ïºR(cBè?€z+Ž;l?kuØÀê?€z+Ž;l?ïãÙè­í¨?vG¹Ô¬Òø?l&tno}?vG¹Ô¬Òø?îصm'÷?Šww¨$™4?¢t©)—n•?Šww¨$™4AGN4FGL J1443.1+4728¿Ãä8èî…H@N&ԀuÀ:k"Úí÷ÀÀ<¡´¯Ÿ•\@r*£Í@^ïCðÙ?¾a¥'°?ÈõæA½å@37º@Ó´Ï*8¿º^-ݳÏÑ¿å¦Ï!»¼"¿ç-O>+´º¿é©ŒUä8#¿ð?ïæþ!¯AGNnlsy1B3 1441+476?ïÝ!DY‡l?p_ÀUÍì?qo]Ҍ^?p_ÀUÍì?ïÙ$¹È¹?ìÉÙ³©%?sm£F¯?ìÉÙ³©%?ï²"-¹³?|FVâøû¯?ƒwtÊ8
/?|FVâøû¯?¬Ë?vú«'™ ?ŠÕ~Q]£q?vú«'™ ?ïœz?iÕå?Œøá2xU?ˆáp/ÙZ¦?Œøá2xU?î`|Ž¾A?´-—åOÖ?©÷è684ö?´-—åOÖ?î
œÔ??¢ ›"YJ?®¾ÿ&2¼?¢ ›"YJ?ë Éý1?®³zóꇙ?Á"Ø;À?®³zóꇙAGN4FGL J1443.6+2515¿ëæK-GXQ@P4t>–=ÅÀ;-ZyɺÀ<4šöå¥@#

éw¨X?û½{Uá³å?Òð'ÿ¤:‡?­•9•T?ð'ß»¼Ú@­pՀ$©¿îÖëÔÏЍ¿ïþ(ßó>?ïû»'w"?Újµ ¶Cs¿Ö£D\¿àŽ¿`}™3AGNbllNVSS J144334+251559?ïÿH2|\¥?b™S
€Ç?ù¯³Èæ&?b™S
€Ç?ïô瀂Fl?cÀðëy?V0þ¦<Øâ?cÀðëy?ïå¾Ã/ü?všœ'ì1?jáAFnëÅ?všœ'ì1?ïõZ…1­¢?K›¦°?UJõޝ;†?K›¦°?ïþzÍYBD?-~oÁ;£g?(S)q+r2?-~oÁ;£g?ïÖÙM	&?Ž¸†"?t"{ÚÛE?Ž¸†"?ïÙ:áÂ?{l É'û&?s~b"žTä?{l É'û&?ïáë0ÔÍç?iւåÄ[·?nÏ0±y?iւåÄ[·AGN4FGL J1443.7-0954¿év¢žŽ@FlvJßøÀ:ÜdöúÀÀ<hô'
´@™Úk›…@\}ÿà?ÉzúÁ»!?p:ÙâãN>?¦¹ÉdãY?þÚÛô#`?¦É{ßto>¿éžÒ¾~Up¿â\~¸+¿àw@Ý?â¿Ö6h½ÕG¿ïúua«ì'AGNbcuPMN J1443-0953?ïúÕ¢o'E?9¿àZg7n?D©v'àAT?9¿àZg7n?ïïFQsA?cúþÁ'-?`¹®­ìþ—?cúþÁ'-?ïíÂau!%?Q˜Ô)ë­?b=ž´*L?Q˜Ô)ë­?ïøäǑÇ?3þ "oê?Loäk†U)?3þ "oê?ïøFæCke?F"Ìp"´n?Näf÷EŒ?F"Ìp"´n?ﭛ¯¦ÿ¼?–"õ_'?"™¡?–"õ_'?ïéÿmUe?p'"†;ˆ·?fénîªØ?p'"†;ˆ·?ï×9ØòR¡?eÝî_¨ô?tc¤cSb?eÝî_¨ôAGN4FGL J1443.9-3908?Ýé30à@2µ÷øʁ™À7ë府mÀ;8˜Ä@\a¾¶ß?ûÃ/zA¾?œ¼åN"ø¨?¬ÇïBmÍ@ˆ®`Ðû0@ í6ϟæ?ïýÖ.u^¿¸ù§÷*ni¿Ûà«;'¿Õ'€áü}¿á8 m]Ñl¿ÓÜ.ÿò¾úAGNbll3FGL J1444.0-3907PKS 1440-389?ïúB••—Æ?E'q)~x?FõªŒ­|±?E'q)~x?ïv€öñ ?"f"3úÛ?‹â_ÂC˜?"f"3úÛ?ï®ä<ˆ¥?‡óëvetê?"Fðßæí?‡óëvetê?ï‰Eµ'$î?v7ªè~µ?®'²Ç(x?v7ªè~µ?ï÷·É§Ë®?RÁÆ8eü?Pl|."ˆ?RÁÆ8eü?îµôv½?·ùüKÑ Ø?®T ¼Ä?·ùüKÑ Ø?ïÀêð	¤?†S»Ü#¿?÷Š¢5Ü?†S»Ü#¿?îI¶ùÚ?˜bö#Æ?«nN¶H0X?˜bö#ÆAGN4FGL J1443.9+2501¿ïÿ¸~ÙqB@P,†hÍÀ7Ðe…•Ö–À;]ˆ{¯¤@ûV$#öª?ÿwÃ Ô ~?—	"ŸG¿˜?¹®œ`w	@!ìæŠ
5@ù$ƒmj¿½¼O?òøõ¿Øó¤·Yô¿ál¹–m•¿á¢9ìN¿æµ6]ŠÒ¿ç_û¹IbAGNfsrq3FGL J1443.9+2502PKS 1441+25?ïöÆı0 ?Qøw捈?RrvÌYo;?Qøw捈?ïëÿGœ?,¶ÆÀä?dæÈ¿õ?,¶ÆÀä?ïqËF1_?'|PsåôÊ?'Æ—9Ô_?'|PsåôÊ?ïüÿ±•R§?6Á{ëO¢ê?8qNr˜Ç?6Á{ëO¢ê?ïíè2,<?YJDã?bóýîKÛ?YJDã?ï§%Æív? šªÝ+E?†6»D¢ƒ? šªÝ+E?︎Cû"?‡W‡_â"?Üog?‡W‡_â"?ïõÑ@$q?LòHa4¤«?T]·ñ?LòHa4¤«AGN4FGL J1445.0-0326¿ëßҋR®ù@Hw @|ÇÒÀ9‡9+
ËÀ;î¬yp@ å"aÎüþ?ù¶ï¶àë?·sJ$'YÚ?»¼LÞRD@Ôƾ•Òe@"N÷3þŠ?ÐÉ@üžý¿æÛ§r$¿ÐúAd¤Dm¿Ðí»Ú·5¿ÒK1­>½¿äv‡EÙþäAGNbll3FGL J1445.0-0328RBS 1424?ïù8Þmß?PñzÀ¶J?K…ö
]Ã?PñzÀ¶J?ïÕ+ç.x?€Ø ԓ?uj‰¶W¬?€Ø ԓ?ï͇ÉÒ5[?z.ÙhXÝ?y<7á'0?z.ÙhXÝ?ïÅƱˆVY?bÕ¤\ú*¡?}§&‡?°?bÕ¤\ú*¡?ïï¿Ì;àß?Xµ—¼ø«ç?`@3ɞ€œ?Xµ—¼ø«ç?ïcÓ/m¬?§rюlY?"…ž4êà?§rюlY?ïrޜƒÿ?1õ/ä?'¤,mçÒ?1õ/ä?ï
ìx"Õ?ŠyàúRØD?ž¢|²§3j?ŠyàúRØDAGN4FGL J1445.2-1954¿ïž½ÜU<.@A¾ýq?À;yåŸ+ªÀ<r`±¿Ÿ@öé·>E5@AƎÅ*A?Á&Ž_(Új¿¶û`‰ÆÕ?öRXâð$Á@Û³'ÎÒ?Ú'Ý¿ŽJÜ¿æCx$Õ¿µ7ýu×s¿ë)xŸN¿é*ƒ–øÕi?ÁóTöÒYÕAGNbcuNVSS J144511-195853?ﻺ«.ŽÖ?³ž"‡ïl?U/ŒÖ'?³ž"‡ïl?ïïè7XÔ$?qSŸÉ»H·?`șml?qSŸÉ»H·?ï·³Ÿ÷y?…;õ«f–O?'ÿ
·?…;õ«f–O?ï÷–‡?9þÜ?¯Ü2?PÓÖoÐÚ?9þÜ?¯Ü2?ïðþxý~?\³ÝÝ×9J?^;ý¾$?\³ÝÝ×9J?ï¼Äþǜ?"ÁÞfh?€ÎþŠôã?"ÁÞfh?ï­âGO9?†»×M?"‡[ñ›ÍÌ?†»×M?ïȗ|š§?l"i$¿y"?{´A§˜Ò?l"i$¿y"AGN4FGL J1445.9-1626?ì#ÎÚKÄ@C(˜ëÀ9ìã.qÀ<õHG@°jœ€ÿš@•öâJ"?·`oA{P¿¡$`©ÛS?äg]Ж@Õ@–ÉÁ¿»ƒk.ø¿é–ãô5ǿ䟗_'œ}¿ä dŽõÑ©¿ì¨þoH?½¤òé.–AGNbll3FGL J1446.1-1628PKS B1443-162?ïû¦µ¦?:ÞÌ;"¹È?CÍd—BH?:ÞÌ;"¹È?ïóƒl¨í?]Ö²Q¿ñã?Xù&@2Ty?]Ö²Q¿ñã?ïâ!Á#~é?l(c/á?mÞ>¬f|?l(c/á?ïýnæÆ%Ç?$'Lrß
Â?4ˆÊm&+w?$'Lrß
Â?ïõ=ÖòŒò?Uˆ.`?U"R¥Ë‹?Uˆ.`?ïË£qQ?}N˜y<´?z.?4¡`?}N˜y<´?ïÛĕî?x9lxpI?rµ[宙?x9lxpI?ïóš×å¸4?N̚ßÍM?XÊPšDð?N̚ßÍMAGN4FGL J1446.0-3039¿íjå6َ…@:
§;BÌ-À:ó"PXÞÀ<nsGyB@õq´ùŠ@趽–Îä?ЯûIaô?Òcˆ»zêØ?ü|MÃØ1…@"Ì€KÀ¿ï‡Š¾4ƒ•?ï¼ë
)´.¿Ù©`J{¿èÕ@8Õ3¤¿ì%ƺd¿Ó/K²…ùªAGNbcuPMN J1445-3036?ïùyÊWÂ?Fv#x-´?JÖ皢x?Fv#x-´?ïïå3S?b3y'ÖØ?`Ìi
"³?b3y'ÖØ?ï0³}+µø?‹Ã‡oC±e?™éW¥?‹Ã‡oC±e?ïùþr¥þœ?3'SŠ;Õ?H5ëiÔ&?3'SŠ;Õ?ïõžA–o»?VèY'´
?TÃ}3U™š?VèY'´
?ï½]Vzé‰?†Ø'ºRMŠ?€¨ªUîçÜ?†Ø'ºRMŠ?î•@{g¡Ç?™Š§KN?¦«øH©üŽ?™Š§KN?ïåc!•?_5V&%?jœßeðþ?_5V&%AGN4FGL J1446.3+3111?×5Ç~"@P)ú—á2µÀ:¨ñ-Õ%aÀ<©Êbh@rÝ4y@Sw[0?À&ágc'?'ùXyœVÁ?ÑÞ¸ù6@û0ÍÓ2¿Ö¾ÔãÄ¿ßâ¼Bô/¿æ"º!N"G¿ì¦á€¸ø¿»ãÆÃö¡¿ïô½±¦×AGNbcuMG2 J144640+3110?ïÿ=u_?|:¥óÞB?ØYHjýó?|:¥óÞB?ï÷ؼø¡ð?Uw§¨±f?PN†Jb#¾?Uw§¨±f?ïÚ¤Zpm?t|ì‹>B?rõ­Ô'¡½?t|ì‹>B?ïÿÓú}>çyÌ,?>ö
Wׯ`>çyÌ,??ïý@2¨§\?92%¶>?5þjV¶å…?92%¶>?ïáiE­£?sr&Hùÿ?n–º…78?sr&Hùÿ?ï¡Á‰€Oy?‰[!‹Ve?‡£[½«?‰[!‹Ve?ïÿxVò"?
%¶N¾"?íïÆl6i?
%¶N¾"AGN4FGL J1446.7+1719?ïÖ'žs-@NÓ³áC|WÀ:²ìzçý«À<s›x¦@Lȯ0ړ@äÖä}Ãz?Ä#-¡?¹zþuÍs?ðítw¡!M@–më?ïá\Üyèú¿àH8³¥´Z¿ì4á=òÿ¼¿×—ÿ»Œ‰¿ë{Háa«¿ðAGNfsrqS3 1444+17?ï÷!™´*?o{¥Ã?Q¼Í¢…?o{¥Ã?ï÷B^@Êm?[
3º^Œ†?Q{CRp&b?[
3º^Œ†?ï…bîá¶?ŒIk1eùe?Ž§DŠÆˆ?ŒIk1eùe?ïõŠÕÙr?= Q"bpÓ?TêUHܽ±?= Q"bpÓ?ïçâ?$Øý?f$!¶Ë»û?hÁàrS?f$!¶Ë»û?ïÍ$Ûyp?¿Üý*?ym'+p"?¿Üý*?ïf1^‹•d?'â÷p4Q‰?"9Ô3´½€?'â÷p4Q‰?ïØ`‹¨a«?cÎ_IÀ¬?sϺ@lÒr?cÎ_IÀ¬AGN4FGL J1446.8-1830¿¸"™Oäµ@B;½‹ç)À;·ª%ÙÀ<†šÜ¸o@ N'?ØÞ?þsŠ ÒH?Óû–
óފ?°-ÜP§?Üٗ ¢‰@—ñ¥]¿è=.ߑu‰¿å©ÊiE=ø¿é¨@[9âz¿¹B	岿ҤvÂT"í¿ïú Ë®AGNbcu3FGL J1446.8-1831NVSS J144644-182922?ïþŠpB?,ÐgCµY?'Xø|¿ô?,ÐgCµY?ïóyAFi?]Ýg©yaô?Y
É*üŽú?]Ýg©yaô?ïíã*åºb?THûÇa(?bÔê+)?THûÇa(?ïþ(#'¤?ÕR'!?-}Ë×x Š?ÕR'!?ïþV"h|c?,™{$ÁÃz?*—¼ …¥?,™{$ÁÃz?ïÃò$9	%?"é˜!®ØC?~îi?"é˜!®ØC?ïéBXv?qy?Ê®Ú?f½ä~N¢k?qy?Ê®Ú?ïõ¡I]¹f?M%^ìÖs?T½m&P¤?M%^ìÖsAGN4FGL J1447.0-2657?ëûÉýQ@=09-Œ*À;‹;26À<—)2ÿ0Í@ °›yB·
?þ³&Ó©_à?Ç£ue‡Ä/?ªugáÏ×?âNæíàBË?þ³a'È?è%¼£n/¿ïÿÿ)@k*?ïÿøsCÄ{¿è©ý·{W¿Ù,ëñUB¿±Ó	&ð.ÒAGNbcuNVSS J144657-265713?ïýâ܃¤?%zú—†Œ?0éÅ
I?%zú—†Œ?ïéÏS?nq{)VdŠ?f0äŸ2}?nq{)VdŠ?ïèÕ©À-W?c?n^?g*VY‰.?c?n^?ïäÿ(?Yô%Bc¯?kpê"›ÿÜ?Yô%Bc¯?ïü\™^$?5_¾ÓÇTk?=RßKÑÇ?5_¾ÓÇTk?￸@'†?'¶ˆ-¶$?€ïÍ 	à?'¶ˆ-¶$?ïëÏD»?lԁ1@?dáð¿$?lԁ1@?ï­:êÑ^q?~Û¹Ô…?"±EK¨cÑ?~Û¹Ô…AGN4FGL J1448.0+3608¿ë5,`õÒï@OÛKƧïžÀ8é™ÛøóÀ;¸˜SH|q@g.†?ù˜Â¤TÞ?ªF-ƒ=Y?¼üë"£C@¸á]}Š@	¸¯&Ëî¿ïb²|¿n??ïþk«IÅF¿Ñ)õœÏ®ÿ¿ÚGž¿Üí:*ž9<¿à®!`¢ØAGNbll3FGL J1448.0+3608RBS 1432?ïãûŒ .V?‹'ÒIN{?lsDTʆ?‹'ÒIN{?î\P<­?¶×÷&¬Uù?ª:þ®œ5*?¶×÷&¬Uù?ïLŒÂèë?˜%Èçdþ‡?Ÿn_ܶ?˜%Èçdþ‡?î'GJ
âŽ?¾@J¦tý?¦Û‹`Ù¥?¾@J¦tý?ï³Ë.ŘÚ?…;CØ.ñ(?ƒ
4^gýˆ?…;CØ.ñ(?éÑ9-­ƒ?Í·Œ5zW¬?È»K­Iò?Í·Œ5zW¬?ïu`2?˜Lë	=Û?ŒQZÜ1©?˜Lë	=Û?é=Cœ·Ü?´–y¼âýn?Ëþñ ?´–y¼âýnAGN4FGL J1449.5+2746¿íŸTª.ð·@OìÏÃøÀ;ÐÄv¼õ¿À<øV6mzW@"ox.åƙ?ô•|3WEa?Ø\Kz§»ñ?Ù]لÁg@¶ÄŸä@µréµ?¾¤çÀîó¿ÝI¼ÈÊ?ïýÐÈÚп¥´£5NÁY¿ÒT9]nÆ¿ÛîH}GS|AGNrdgB2 1447+27?ïêÊv†D'?bt' —iÝ?e5‰«68o?bt' —iÝ?ïâù›8†?J&yòKk?mdÿ¤1˜?J&yòKk?ïpuÆ"0#?‰
•;XI,?'ñG@áe™?‰
•;XI,?ïž|Úñþ‹?uê­ºæ(ê?ˆ`É91‰l?uê­ºæ(ê?ïÙÆÓÂ?o`҆ª¾'?s–4ôw5?o`҆ª¾'?ïÂևiI?¡rÃ܂/A?‹ÏJSÖÙÐ?¡rÃ܂/A?ï‡X€cs?Šu*šŠç?Ž)ßÙa35?Šu*šŠç?ïݧ¡«G?'b>hºa?œdKZû ?'b>hºaAGN4FGL J1449.6-2137¿ï²H#±@@¼Èÿ¸²dÀ:»I»4ôÔÀ<Kžã…uö@çk´"@eäEVJ?Â-`‹[¿«9s'óS¹?ê†nCªz@Òùæ‹dο×ÈçDÈ1¿âìÊ-¶°¿ìÉv7]d?±å/D;CM¿çRw@Ý@¿ïÿ‰XAGNfsrqPKS B1446-214?ïþY‰ÃÒ? ÁdòÈ?*n£ë[D? ÁdòÈ?ïó©åŽ‡?Z$»ƒf	?X¬4•ú£Ù?Z$»ƒf	?ïë8ÇÅ?a¡ßÌu8?dÇ90ÁrŠ?a¡ßÌu8?ïÿE€Þ$?Û°oI
Œ?P'ÎNù?Û°oI
Œ?ïü3Lªö?7Áýð ??¾c³'ç	?7Áýð ?ïÌ£Úî¬#?}e÷ÞÏÕÕ?y®¨FV6?}e÷ÞÏÕÕ?ï×Î{¬&m?x	ǁ5W?tÂ
¿ýÐ?x	ǁ5W?ïüÃqs$?6êž[Uª??¡æP}Œù?6êž[UªAGN4FGL J1449.7-0910?ï+RßJþ¬@EÞB||RaÀ;)!°:À<‡àmòL@ >1´Øå4?þ‡S–€	¦?֝ţ7Ó?»Ž-TÌàï?êð äÑü?ìæ¹ÏçV¿ì§'Z¸³:?ïþ¡€Ã´Ë¿êéˆÅ5ÿ–?³=ïϱ-µ¿ÝÐ$p!Ñ¿ïÿÏ=ÀTïAGNagn1RXS J144942.2-091018?ïúqwUeÒ?TÁ! +?F:!ڙóO?TÁ! +?ïd~Wô?›èÂéÍx>?"p5# ·?›èÂéÍx>?ïoÃ\ös?âàŒ&§?'ù¹?âàŒ&§?ï¥[ìåÆï?q¥D7ß_·?†©¿¯Z?q¥D7ß_·?ïù?7$ò?QX1ÔÀ4"?K#[˜tk?QX1ÔÀ4"?ì~Ê榓?ÂÛK€1È?¼	¯@ÊËk?ÂÛK€1È?ïsҀüûÐ?Ïā'T6?'…¯å‡ïþ?Ïā'T6?í:þø~×?¥äBÁ7ñž?¶((<	F?¥äBÁ7ñžAGN4FGL J1450.4+0910?îçÚºv3
@LT°ò{²ÿÀ:7s	â×ÑÀ<e …F%~@´—Â;ú@æ3
9?Ã
'åÍúŸ?ÅëX¦4]@&¤û¨'@SF¶È©}?ì!åbÅÇö¿Ù8¸ãá¼H¿åÍà¿åq•n'¿é{NP¿ïìŽ:AGNfsrq3FGL J1450.4+0911TXS 1448+093?ïêáRôLK?h&ð"_ê,?e­r$²?h&ð"_ê,?ïóº0@S?esJ§zw$?X‹ÿ95?esJ§zw$?ï¡QÿÅH?"NµVûÅ¢?‡«¸u¿Ú'?"NµVûÅ¢?ïó‡o±¤ä?B8íèq9ü?Xñ ²³·?B8íèq9ü?ïÚ}k'I?o†–Ò)¯?rÁ}΋ã~?o†–Ò)¯?ìñ'?¶'!%¶?‰¾ÕñÂ-?¶'!%¶?îâhP)×?˜wÒä,Õ?¡Ùzü'»™?˜wÒä,Õ?ïà" ˆâ?\g/Ŏ?oçlð>?\g/ŎAGN4FGL J1450.8+5201?Öùd•<#@LEåóöÀ9¯UªLoÀ<P)µ/ë@7Ž`U€:@ ÷üü??¶2¬`×ÂZ?¼ŒÛ›Ï¿@5 üÏÊ@£þ·Öp?í/B]r¡Þ?ÖؽÜD"¿ã&??#€¿á*™Á²'d¿áÚŸ‹Ëü¿ïÿú÷''ýAGNbll3FGL J1450.9+5200SDSS J145059.99+520111.7?ï÷ùÎã}h?EY!±s™&?Pbk™'?EY!±s™&?ï Boˆ›g?")øô^f\?‡ïd!HÂ??")øô^f\?ïÒd"‡¿…?}`QpØR?v͵´'~?}`QpØR?퀭–?–Gí†T
6?±ï»û~Ì?–Gí†T
6?ïÚ)y¡Á?r)gšÍ?rëC
Ós¡?r)gšÍ?&w|Ó?«!íƯ‹Ð?¦Vݚ@Î?«!íƯ‹Ð?ïT5Çb)Á?"¨Ìu5¢~?•yGùê?"¨Ìu5¢~?ç¹)ž×=‹?²ì7KEΖ?Ѝ¬ÂQ"é?²ì7KEΖAGN4FGL J1451.4+6355¿ïÚÄ'.:@H:A€ÓÏöÀ:ƒŠc›±À<¦p‰Õ×8@ "6}•'?ýNQÒÓw?µxõµ#bÜ¿€ÂZï
®?Ì©3€
&u@à±F?ækҁA³ÿ¿áŒ&ÿÉ#u¿ß S<h5¿âˆéH-–;¿Å€¢è!çܿʹÁáAGNbll3FGL J1451.2+6355RX J1451.4+6354?ïþï`d]'?ë"ñ4‹?!	ùl?ë"ñ4‹?ï÷S;;jd?T+Җ»Bâ?QY‰Žª—_?T+Җ»Bâ?ïöߔ‹Ï?eÑ!}££Ä?SúAB1?eÑ!}££Ä?ïþwÙo6]?'s!¿™?('f6ì¬`?'s!¿™?ïþ D2Ò?,káé6?-û¼N[?,káé6?ïßkœŸø?qyúj'?pJ1šqù?qyúj'?ï÷ãL¸b?d.ëŒ?PÄ9!×¹?d.ëŒ?ïý½šÍ?(ù±mX?7oŸö3æþ?(ù±mXAGN4FGL J1451.5+1415¿ÆÄÀ†9âÇ@M›ÑþdõMÀ:ˆÒÿì´ÊÀ<wí4Ka'@'{yž@ݖÁxô?Å{>û…i?Ò¾ä!'B@²• Ž@ë¾(DAοî‰þñã?·Ð³Œ4c¿åGªfpw¿èOø ºÎ¿àLèyÑ¿ïÿçvœ>AGNbcuNVSS J145126+141626?ïîK*SnE?\h©Ètþ!?a´Õ6ãŠ?\h©Ètþ!?ïê"Ö¼9Ø?vqè‰Æ"¶?ek)&ép–?vqè‰Æ"¶?ïD0þ¤?'™üê?—|Yøó"?'™üê?ïÁÿ£R™Å?ehUÞg¬?.YrÍ©?ehUÞg¬?ï݉#Ä?s,tõlË}?qø4ŽåÒ?s,tõlË}?ïcã",X?›óaà»Y?"Ãš¦ø?›óaà»Y?îŒrÏ!Þ?!¾ ÷øC?§8Ó
7w?!¾ ÷øC?îV2	E+·?•,Œ+ñD?ªœßn@ù?•,Œ+ñDAGN4FGL J1451.8-3851?ì;—±É!ƒ@2FìÔªÀ;qߐô¯jÀ<‡ªhô¶ @ þGG<Tš@gã'ñ·?Ì+ýß¿BÌ?{E"ï¥1?³\&á/?@Ùt·b}¿¦<!•.®?ï[›fù3]¿éÌewS¿Êz:ßO¿ïÿüÚ±'Þ?ïÿíÁ9ÔAGNbcuPKS 1448-386?ïì¤Onìâ?cn´¼&`¹?c[°WY®Ì?cn´¼&`¹?ïåðš¡?reüZÅM›?jâ†[%w?reüZÅM›?ïAt?B?'ZÒhÕó?—Ñ}¯¯åÉ?'ZÒhÕó?ïò5iÄ>ß?KL¸ç?[•,	ŽÃ)?KL¸ç?ïß4{ÒE?p˜Fkrâo?peðÆ6e¯?p˜Fkrâo?ïVW³ßÛ?¤ t0~x?•<µÌ6¬?¤ t0~x?ïuÞ¶P«á?Ž¢ûƒs±`?'D)<É»Ê?Ž¢ûƒs±`?栗ˆ×Õi?|H|vk<Ê?†]×ɍ?|H|vk<ÊAGN4FGL J1453.0-1318¿ì¨¾ôƒ0]@CøŽ£œQÛÀ:Ó Z8[À<Zê'-@Ô®¯Um›@^pc?jy?Ä:šE;¿ŠðÉZ7À?ÅçúîHH@ñp;Ò>&¿îPáϓPª?ڂRÀ—4e¿ìJ[¾l·¹¿Î0CÐí¿å/5B,P¿ÌT—œiW²AGNbcuTXS 1450-131?ïð7¤BPC?œàI§'?_¶ô®Ë(?œàI§'?ïñð£Ÿ4—?^6"ýzr?\¹2?^6"ýzr?ïރãÎ(?q2"Ѝ'?p¾qŒ0?q2"Ѝ'?ïüËÝ[Ù?#œŠVk'I?9¡ø±ub?#œŠVk'I?ïê:ç×?dš;´Bޓ?eÅqü¬o?dš;´Bޓ?ïÇYz/?g4¼¨ù?|Sxr4?g4¼¨ù?ï´éÛó¨¦?‡Œ¦:Ñ]?'ňý>€?‡Œ¦:Ñ]?ïêb`°E?Yò'…‹‰"?eŸó°ÓP?Yò'…‹‰"AGN4FGL J1453.5+3505?âÓ£ç·@Oeì,äd™À:¸ŽS™ÛÀ<µ™ÙZyÉ@#>Wÿpc@X*™0¾?ÄeqH턨?²´rˆ2¿?꿹SsD›@Z(*¨3?ã¥L?ə'¿æ]4Ä,ë¿ä½Ø"kdÓ¿á»2Ál"¿ïæõ½†Þ¬?ëñø¶Ô"AGNfsrqMG2 J145315+3506?ïü×7ù…V?NžÍ;ã‡ã?9FBGÿ0°?NžÍ;ã‡ã?ï÷ÀaÀ €?UÆZì¯q?P<†þY?UÆZì¯q?ïÜgxÎâ•?u"'æ4Ç?qÌCƒñ
_?u"'æ4Ç?ïüÒ±«M?(†¢Öþq&?9o´Ø?(†¢Öþq&?ïý¶íÌ?/JJŽÎc»?2H–
Ç«?/JJŽÎc»?ïÙÏ‹±O?¶›÷ª«?sp§™tÎ?¶›÷ª«?ïãȯå>?u¦[H£üU?l7PcW­?u¦[H£üU?ïö·.?Gni¾ Œ?Søü°4+?Gni¾ ŒAGN4FGL J1454.0+4927¿ïãݘ›Ê@LÉÛ"Ðå`À;Lë8ȞjÀ<ª"Y–tK@"…|V'@¶LãÞa?Ó­Cðo¿?Ñ#l`üD4?ùìúÕÔ&@GÍ`Æi?ïõðaýK¿æÒ¬X4õ¿êÕï ·E&¿ÜjÃQ#¿ïñ'L ¿ãÈÏFúTAGNbcu87GB 145232.0+493854?ïöìè¯Ï?Nt_Á^@?R'ü
ärÎ?Nt_Á^@?ïîÝK}µk?a)¦´¸˜ˆ?a"´VO•.?a)¦´¸˜ˆ?ï´¬Ñ@
B?zvJW7¯z?'ÔË´tíb?zvJW7¯z?ïÑC¢t½?^|šóí?w^.å=Øc?^|šóí?ïøÀÞNw?Pu=¦uv?O ýu^6œ?Pu=¦uv?ïŃèWlÎ?{m†»ýcò?}>è7Tµ?{m†»ýcò?ïjbŠl]ª?Ži…Þ.|ž?'³®´,Â?Ži…Þ.|ž?îÅ`¡¢Éæ?© Òçc?£©õêä"?© ÒçcAGN4FGL J1454.1+1622?îÊb		"ý@MÒ*¡"9ÞÀ9ÞúŒ"¹À<Zjۖ"@OÞÉ# @T[òoÅ?»Ð 쉬?Å`€Þ·°Ü@žÒ¾~Up@©§°Å?í>aå£2¿â¶œLÒA¿ål(—9¿æ:m"gÙ-¿ëæíª'æ!¿ïýÝÑ×ÏAGNfsrq3FGL J1454.0+1622CLASS J1454+1623?ïéMc,—…?hEÚK/?f²œ¯¬‹#?hEÚK/?ïé["-ýr?t•ðîCW×?f¤kª'T?t•ðîCW×?ï°…Ûˆ?®ç:Š‹!?ƒÿ|쟃ô?®ç:Š‹!?ïtæ•åsÑ?vÓù­þ›?'c-CQ…Ñ?vÓù­þ›?ï{t:Âý?ŽB	¾.t>?'x©X*C?ŽB	¾.t>?ï£Á­¬B‹?÷_¦uˆ?‡""ï]=?÷_¦uˆ?í—&? W¸m'*
?§G$Öï¨? W¸m'*
?íÉ"èږÜ?˜[d£?±¶èºã?˜[d£AGN4FGL J1454.1+2647¿¬4à³8Åý@O[2ßP]À;,7–oCÀ<°ÛE5"7@ØâÇàÔÂ@çÔÅ¿'R?ÆÛ Ña?¤Æa½y?Ù.$Àÿ?óT³.@?ïÉ,.\4¿º–ØÊü¿ãp,¸Å¯¿ãd¤úö«Ã¿ã îA灿Ö÷u'c/AGNbcuB2 1451+26?ïâM7@^?{Ž ԈÆI?m²Èæ‹Ã?{Ž ԈÆI?ï«Ù–E‹?ŽÎÆÇkX?…	škMAW?ŽÎÆÇkX?ïs¯Âg?ñ}dBö?'Š¿âº'?ñ}dBö?îɏ;ØÚ]?†"6¨áõ¤?£gA–s+?†"6¨áõ¤?ïÉ« ŠØ?}e–Äð?{*/¾³~M?}e–Äð?ív°ó
²?½FÄ=9Ïã?´JCyp?½FÄ=9Ïã?ïbôJY?'§>€•Òë?"¿a{ÜI‹?'§>€•Òë?éÃdš¹Í?¬ÅþwJ×m?Èòm½•Î?¬ÅþwJ×mAGN4FGL J1454.4-3744?§—Eb|û=@3ÄüóÀ9µm¿öûuÀ;Üz¤áÌ8@ Ç†>@Ñ÷" ³Õ?ÀVË~C&ñ?É«ÿbKN³@ؖdZól@cô?ïê<´¼4Ï¿år†?tµ	¿æƒþý¡€ï¿çñLÝÙ¿ï÷Œ^G³ô?ïeÞ×sAGNfsrq3FGL J1454.2-3751PKS 1451-375?ïætw1v?l/;¡ÕŸ?i‹‰ƒ¿Á?l/;¡ÕŸ?ïàî
›J°?xóQ3ñ?oõKø @?xóQ3ñ?ï'ïÏíNß?…\˜DJ€Ù?DöíØl?…\˜DJ€Ù?ïô-£É•­?Déw¦6ÇÁ?W¤¸±ŒÕf?Déw¦6ÇÁ?ï˅"¹¹?'°ÁüÖª?~:=-ÔïÇ?'°ÁüÖª?ï XaYÐñ?§R¥:øÕ?›ôóÍæ©ø?§R¥:øÕ?ëñKÑÜùb?­8/ᮬ?À:иŒw?­8/ᮬ?ï¬Rǀ»/?uѓ¹æU1?"ëN£([?uѓ¹æU1AGN4FGL J1454.4+5124?îš1i•¬@L9Âã>ÿÀ8«]|OÀ;pêWøš@"3¬?ÿ~"Ô]ºÆ?—Ù~¥¼+"?¬f¸#{ï@¹¢ž%•@ô½:ˆ'
¿Î4
H®D¡¿Úp.›ô½­¿áßÀà/€ ¿ÝâÉc`Íu¿â‹ÑŸÅW¸¿ãë[-M@AGNbll3FGL J1454.5+5124TXS 1452+516?ïûAÍ)éÞ??r¨ŠŒ§a?BøÊՁù??r¨ŠŒ§a?ïòFýэ¸?aÝçïÃgã?[rgãP?aÝçïÃgã?ïâ4u}…'?rƒó·i°•?mˊ—?rƒó·i°•?ïûb@*×3?2Ro%*hÎ?BvþiäKè?2Ro%*hÎ?ïü…‡=÷\?3Î=í؇1?;ÓÄÅQ$Ç?3Î=í؇1?ïÒD˜,Ôl?€L'ŒØh©?vÝ´b½ö?€L'ŒØh©?ï⟆\iÒ?zkþ‡®*b?m`ytÛ~&?zkþ‡®*b?ïóø
 ±?I0J2ì•?Xå–ÁNÊ?I0J2ì•AGN4FGL J1454.7+5237?ÀqÚ¡)c"@KÜýŸÓo~À;=*³1ñÀ<Ö»ÉoJ;@
—Éà´5?üË;¸<òÐ?Ô¤Kc֔!?ÝuX<8@•0¸/@9Æ7‡UÊ?ïÚ6ýÃÞ¿ín_E°¿ÈÒ<ã¶^¿äÍ _Š¿æó|†¿ïÿû˜'2AGNbll87GB 145311.3+524904?ï𥨁Ð?W¸yÞI?^´¯…ÐJA?W¸yÞI?ï×Êño2?tˆÒœÑz?‹Ê
Jƒka?tˆÒœÑz?ïEcLÎ\?‹äìT…?—SŸþý:m?‹äìT…?íڐŠó'?£Õ•oÔ©?±+Ñð˜Ç?£Õ•oÔ©?ïÎJ9ÎǓ?}?9G‡?xÚã&Z¦¢?}?9G‡?íŒvd?¶©õBð}?³Ÿçsmä?¶©õBð}?î\ð0Ìs?Ÿ·©çÿßó?ª?>»Ê?Ÿ·©çÿßó?è?ÁC8?±ˆJÀšCË?Ïû®ó¯ ?±ˆJÀšCËAGN4FGL J1455.0+0247?èÊôŠMm¾@IÜ¡ô±îÀ;¢oþDÀ<ϓ¤£@ ïþ¾âSr?óDƒ½B(?äF
<ã?ïýfÞ"N@dä]ã
&?ô†²+‹Éø¿ïÿ¾ýq??ïÿò~#¿?9Ár%·I®?ÖúÿšÕXâ¿á*Ä>³Äé¿ïþÔãÄAGNbll87GB 145233.9+030210?î‡p«Jg?Ã#|LèÍ?§ˆõMóž‹?Ã#|LèÍ?ë›AÈTö…?ÁgDGW­f?Á'øÞ¬%ì?ÁgDGW­f?ígRÑwñ?¥ßáx;·!?´ÅirµÊ?¥ßáx;·!?촒¸m³ü?¢±æÊ'j£?º[j<'`?¢±æÊ'j£?ïñ-À-?o¬ŒÒj']?]Åätf ?o¬ŒÒj']?ä—­¢:'?ÒI[Âã-Ñ?ÖÑÞ¤»‹²?ÒI[Âã-Ñ?î?úꉯ? Ð ÷ì.?¬Q^—e? Ð ÷ì.?æšËûc?ÀOÅbþ°}?ÒËÌh	9÷?ÀOÅbþ°}AGN4FGL J1455.4-3654¿àúA-á~y@3£åÙä"À:K°¡šÀ<Ž`€s@±®MÛ«@ç]<9A?ÁPrß­?™Ôco. ?ÙG…5@èe{.õa¿ê6Ù{0øÆ¿ã'^aŠ3 ¿é©?^º z¿àþ壞U¿ÝhÚÆ_ ¿ëš	`ÑÑïAGNbcuPKS 1452-367?ïûn¶A'?8äYTR?BE'd"ü?8äYTR?ïé1ÞZ¤ø?sP¤*̽?fÎ!Ø5?a?sP¤*̽?ïëܝ'å×?bî_¡Dñ?d#b…Y9c?bî_¡Dñ?ïûmEõúæ?*²ùÍ\hG?BJçÐi	?*²ùÍ\hG?ïéøМ÷-?d[âE"??f/JK¢É?d[âE"??ï‰íö×Ñý?–;¬ÈXE}?"'F›ä°?–;¬ÈXE}?ï·ÖŽ ÷?" A›ƒ7-?'
\HÙú9?" A›ƒ7-?ïÜÉIŠ?d×VŽ+ç?q›[[µyD?d×VŽ+çAGN4FGL J1455.8-7601¿é5îñ(»zÀ-ñk¹Œ~(À:ÞUNæíàÀ<ß®PàÃ@ ¤£e BÖ?ýóžÈ­ƒ[?ÆÛC]!ï?¿–ºÂM¬?óËg†ø­?ýÞU·¿ãLÀmBùz¿èYõ_45¿ÍáS¨c¿á¤Ó‰p#¿Óz­%²Z¿ê>¨çë6DAGNbcuSUMSS J145543-760054?ïþ-È:@ï?vbÝ¢";?-#~4»Tõ?vbÝ¢";?ïîé_T¤G?`'t:ªÍ?a ê"ˆŒ?`'t:ªÍ?ïñreš…õ?T<'¶#7?]5+)%H?T<'¶#7?ïñ=Er·?BfS6-?]…Õ8¡r.?BfS6-?ïúR/çh?<׺ù¹š?F·@x]
O?<׺ù¹š?ïÊdµ1?€:Jü?zÍôæâ?€:Jü?ïìÛÉÑ?r±Ù°xÁÒ?c$6ᙦ?r±Ù°xÁÒ?ï©bœNÍ?wÛGÇmÿ?…§Xåm"G?wÛGÇmÿAGN4FGL J1456.0+5051?ÇnPtÓx@LG¾ýqÀ;n=þhPÀ<œVœÄÇE@ ÿ‰ þ@Â%ĵ§?Ç;«&ß½À¿§°ÉáàÛ"?ä¾4^'J@JT·è9¿ïý»íx;?ïþ
A¢a¿¿ãARz÷#¿ä81¿ë'á¿ã¦">eìC¿¸,+×õAGNbllRGB J1456+508?ïüú(œV?-ðšÕá'½?8/x§²?-ðšÕá'½?ïéîՆ?i3¤÷3'G?fëý+?i3¤÷3'G?ïè¨j9Q'?^_÷¥&4Y?gW•ý¨˜Ø?^_÷¥&4Y?ïÕ}á_ßl?a®/#iF­?uA[¾õÐ?a®/#iF­?ï÷Cý`?M("žÖ84?QyÂZvLÇ?M("žÖ84?ï…1-R&F?›noà'ÆO?Ž³´¼¤zb?›noà'ÆO?ïåÎ@óú?sރ[O>?j1¿#™­?sރ[O>?î•21*š]?™Ýõ3á=?¦¬Üéæ¾/?™Ýõ3á=AGN4FGL J1457.3-4246?ìGً!0Ò@,¦‹¤ôÀ9'Pi¤ßHÀ;ú²÷8±!@4&Œ[Ãu@A¸œ"Ý?³ïîÿ–gz?¤®
aOG³?ì½7Σf¢@N%zãËí?é-¹a5$$¿ã]Ûèɂ•¿è¡ð€0<¿ä±¾>¶ì¿êhhŸ%Ë?Ëgbû!ôÇAGNbcuPKS J1453-426?ïü|A¼Z[?NïAe0©C?<ðfx¢=?NïAe0©C?ï露­?yaæm;{"?f€c+;V?yaæm;{"?ïÞ-ý`µÅ?u<ŽÕ´?pé?&ý·?u<ŽÕ´?ïÿÉۚ‰È>ïh¾dêÆà>û?SÁ¢Ã>ïh¾dêÆà?ïüVr0'?8¤:‹,ö"??uMÖ	1?8¤:‹,ö"?ïkZ'%dœ?£øþ:x?'"­»Sl}?£øþ:x?ï÷©"Ñr?µÏŸ­âS?~$+<ö~Ã?µÏŸ­âS?ïÿ "Ž?e|m˜Ó«?÷V•A?e|m˜Ó«AGN4FGL J1457.4-3539¿ïüEŠÆ@4‰"àÀ8(¨(÷À;œÏ¥©r@f'ÿ"Û@fö^–ŽL? )¢].ü?ÅË3²Ù‡@$·ëО¥@ÓH{ÄÇp?Õ/F߸aÜ¿Ýå"ä±oú¿ä•ï ·E&¿åȖÝ&·¿ëwöaÍ¿êO'‰²›ÉAGNFSRQ3FGL J1457.4-3539PKS 1454-354?ïd–qéHÑ?Õ`Ûg8V?"m1ËmëÛ?Õ`Ûg8V?ï–Rd¦È¬?š'&X°ûs?ŠkfÏnœÿ?š'&X°ûs?ëímnjN¶?®¢6åñì?ÀJHáÎÅ(?®¢6åñì?ïúѦaM?G›²¬ë?D¹et |<?G›²¬ë?쟃‹eNc?³üçÄ5S¾?»ã¤ÕŒå?³üçÄ5S¾?î­
¥û?»ÃUeô6Ú?®u/S–X?»ÃUeô6Ú?ê9ñ‹Ñ"?²-+›ßü?Ç9йÉî?²-+›ßü?ïÝëᘔj?ivÁÎpœ?q
Jc7?ivÁÎpœAGN4FGL J1457.8-4642¿åé*ó7‰s@%©fàé´À:ôé¦ÙÀ<\E–F_@!¡Í­?ÿ_¥'(^?ÃÄÿa©¿¡I÷šÖ°{?ÛÌsvaÑ@ž™ÔÒÖ?ëUë#Ïèá¿àtÜ?,f?I\ÈWó¿Ú×7‰Úõ¿ç@Z˜ÒÊ=?Ðßn"¤AGNbcuPMN J1457-4642?ïüþ»(×Ý?/Çecæb?8
'y«7ˆ?/Çecæb?ïÛö˜Î¦?{È.""'ý?r³Š…ÑM?{È.""'ý?ïï
Mæp?cÓpºY+
?`òþ—ü‡º?cÓpºY+
?ïðqࠜÌ?Hó74ì'#?_>ÉÅ(?Hó74ì'#?ïùÌxä©?Dyn?ž‡‡?Hϵ¤Õ8?Dyn?ž‡‡?îÇgJðqË?²}vÎwÆ?£‰‹OAP?²}vÎwÆ?ïà•ÀWY¿?{]ãh£5,?oj?ÍÂ'?{]ãh£5,?ïÇUÎ((?kxÉʦç?|Uqz¯\C?kxÉʦçAGN4FGL J1458.6+3722?ä:› @N°hÂa9À:@±gìxdÀ<'¤@¼ˆ²@šD7guZ@§À£Éž?¸¦8ŽfàŠ?«ÎoU®2?ñÀgc¼h@
TœåT¿ê7ž&ò¿Ñ¼J^H¿á‡ÿ¨Â+‰¿ä'Ôôó¿Þ@°ÿç¬L¿ë4o©GhAGNbll3FGL J1458.7+3719B3 1456+375?ïþg˜%âN?k,þŽ?)†~"¿Ÿ?k,þŽ?ï÷%O^¦Ã?UŸÊÕ¸™
?Qµa¾dhÛ?UŸÊÕ¸™
?ïðYl,ùÞ?b"¸û[ðà?_M'׆£k?b"¸û[ðà?ïû`¢Æر?,¿5V‡½?B}u°?,¿5V‡½?ïüäz­4?<ºÄW€??èÚÕ[?<ºÄW€?ïÛ$­£*¬?w÷—Oä+?rm©:V?w÷—Oä+?ïîo,]?m1mm¼%?aoÙo+?m1mm¼%?ïòçøŸB?J"&?Z0zŽìã?J"&AGN4FGL J1459.0+6129?ì=É9DoF@HÊnÁ~ºñÀ;NéH-–;À<ïóŒT6¹@£À"'Œ@þú¤vln?Ã¥tU·B¿š³ ,Áæ?ÔçñìA[@$»]Ž¦?áú¹¿©Î›¿ã1bV}¿å/áoA¿Ü˜/w便êŸWH¼1t¿ïêøÒU-AGNbcuSDSS J145852.69+612813.8?ïõ–Šù÷0?Iàñ¶ß­?TÒ飝€?Iàñ¶ß­?ïðÔl1	@?c¤/
Ò?^W'd4`?c¤/
Ò?ïÓ_Ðá?qÐ,üT{?vP~SKD?qÐ,üT{?ïÏùÉÉÑß?[ŸRº8Ö?x;cd?[ŸRº8Ö?ïÝ\ˆÛË?dýüì?qQ»u=Å
?dýüì?ïΰÏì?vÕ¾©?x§—óJÀ?vÕ¾©?ïÄÏ£ýÜË?'ÚÔ¼B¥?}˜.?¦<?'ÚÔ¼B¥?ïmÏ
ñ?‡‰ª¹&§µ?ŸòF&ÓÓ?‡‰ª¹&§µAGN4FGL J1459.0-5353?è‰ù"Á @Ú\ØH+À9½òJ·À;Y^Sô@§ÔNKg‡@Ն¯²
?ºÒ]Ÿ1Lî?Á$xFÜ?ò͗b‡´•@<Yÿ$㺿ïøe˜º?ïû
H5#¿ãší!*È¿êµg £#0¿å$WÞ8Z¿ä"%B{¦AGNbcuAT20G J145935-535047?ïüȎµÌ?<"9j)ž?9»‰Ó-Ý?<"9j)ž?ïÂ8‡l?˜	''Ã,?~ã¼_7º)?˜	''Ã,?ï=·¨ù3?"°3Åòk?˜I
àٟ?"°3Åòk?ïÝrÜbäH?Yă88(?qF'ËÎ+é?Yă88(?﬐Ž¥l-?‡IԒòi?"ÛÜ`óÈ«?‡IԒòi?íí!DY‡l?¸D?¹]Â?°–õÛéê"?¸D?¹]Â?ìªÝ\€Î?¯Ú³öT?#?º¯ùŽ?¯Ú³öT?#?îÍY6ýî?•ó'Å{0?£*l!à?•ó'Å{0AGN4FGL J1459.5+1527?痚»ØˆÃ@M
AÝ!êÀ:ÿ@Iœ+DÀ<œÑ*)Ÿ6@*èãXÕ@Â|ò—?É2.3o?¹y}†8ê?ñ%õ'^éš@p½Úìu4¿ê¼$ô?ï‰ñ Á¬¿ÐÏ(œ¬Hž¿Ü^IA<‹L¿êÙ8¶)ó¿ÔvOýï.¡AGNfsrqMG1 J145921+1526?ïü"Dè^Æ?6J9‡ÜoÄ?;]ÙP_u–?6J9‡ÜoÄ?ïôÑã"k¬?^·,Œë«?V\8s7§Û?^·,Œë«?ï£ËMpª?""7]xüÍ?‡
 3ƒ
‡?""7]xüÍ?ïäû^I{8?QÎuyjÙI?k¡¯¥?QÎuyjÙI?ïúØLC
Ó?BTmn±!??DžÎGÁß<?BTmn±!??ïºp"ªý£?‹'×çÆ
?cÞå¾·<?‹'×çÆ
?ï¬*TV2V?ˆ¡‰?=ß]?"õjñR¢–?ˆ¡‰?=ß]?ï©X'¥£?{Fèõ¿Ž?…©þÛV—*?{Fèõ¿ŽAGN4FGL J1500.7+4752?ëÆGf­è@L¶°hÀ:VL¼q4÷À<Q¶3-Sö@)´½atå@‰‡á
qs?Ä<37
à?ÁƒxǼî?ûúí!*È@|è7"î?áV.	þ‡¿äåܝû(¿âØr‡ÜØ´¿æ- í¶Q¿êÌ_iœý¿ïþ·`Sý®AGNbll3FGL J1500.6+4750TXS 1459+480?ïáºã|x?iaîIV°›?nêE(â ?iaîIV°›?ïǨ'•On?€´Å
öc?|+·>÷0Ö?€´Å
öc?ï»pâsÛ£?~'ˆ0l*µ?#ÇTBÅs?~'ˆ0l*µ?]‰aØ?…ýÔÙ@
£?¤–º'iâƒ?…ýÔÙ@
£?ìnoWë?¸"¤½Â¡X?¿$t…@¥?¸"¤½Â¡X?ïVеÿE?¦‹Igۏ?Ÿu%쯳e?¦‹Igۏ?îpù°c=E? ÆÃ{Áø?¨ðdü_à±? ÆÃ{Áø?èλ0år'?ª'Òlî?ÌÅ<j5ö?ª'ÒlîAGN4FGL J1500.9+5528¿Ð+"ÁÐg@J¥éᰉ À:ä¸qËõ6À<¹ªYÛ=©@oœÅóë@qޟ]'ù?Å06(°ù?ÂA!"µ?üê®ñð@#zÉIàt¿ïôL7å?ï¥~ª*
–¿ß—ºò.Ü¿ÜÕR'XàA¿ëó×"f1b¿Ó$e$œíaAGNbllFIRST J150106.2+552750?ïø'Ò™Ú ?IÃ#B&Û?M´µoèìØ?IÃ#B&Û?ïè¥bûwÛ?hÑ™X°ã?gZ<Ἧ?hÑ™X°ã?ï'¥bá³?…4މ+Æ?‹`–‡f?…4މ+Æ?ï™ýïsr?m84Ùd?‰€"*䳈?m84Ùd?ï±l$ ?ƒh¤Åë?ƒ¤÷Ždß?ƒh¤Åë?ï¢qÝo? µmÓ ¯?‡ycÉG
? µmÓ ¯?ï=¤ùt¸?"(ûŒê?˜K`Ñ|	?"(ûŒê?í÷d!ßñ?¡	Á™8?°DÞòJR?¡	Á™8AGN4FGL J1501.0+2238?ïûÚŒ«
@N,ý\·ûÀ9Å㤀À;ýåﳁ¢@úÌx"n?ÿÆ·	)?¨Ì7Tüº?­@
ÿYß<@3Xz™@ÄÓÏöLù?Õcä`è"¿Ûžœ7ً¿Ý©aùDO¿ß¨"í8¿ã
O¿…ç`¿á€`•AGNbll3FGL J1500.9+2238MS 1458.8+2249?ïýÙ>l™©?!Í3o|[‡?16Y
Ÿ?!Í3o|[‡?ïõûÁú-P?búC@o"?T|y˜àF?búC@o"?ïðÑo&‡?VlY§1£ä?^]!ÎnÓì?VlY§1£ä?ïñ)4Ï?J;¢!8?]­–ÏÛb ?J;¢!8?ïüpM'Qs?3Cƒÿöà]?<}"ƒqæU?3Cƒÿöà]?ïÌ{3'Ó?‡"0ß?yÂf_b¨?‡"0ß?ïæÑ|"Õ?r¿€¥*I?iæ.;Âé?r¿€¥*I?ïäG÷ Ă?["-Jb8'?k¸ê:>?["-Jb8'AGN4FGL J1502.5+5552?®‹ëúó"b@Jo…¸QìÀ:_sN¬5~À<}}Ž¡@…×x¢S'@ú <¶i´?¿0'ùD?Ã=ñÓ'é@ 6^`Þg@P±šÂ?ÏݪÀˆpÒ¿Ýz\9â$¿çEb¹2¼¿ãecœ‡Š£¿çªs;`ÿ¿ïüç|{{¡AGNbcu3FGL J1502.2+5553FIRST J150229.0+555204?î¿
%Ù?ÈKͱ¬¾m?¤.:2ÓR?ÈKͱ¬¾m?ïõÄ{«®*?UçúÍ&"?Tw3L?UçúÍ&"?ïΊÓÓZ?ƒ²Ç"øØ5?xºÀø$?ƒ²Ç"øØ5?ïó‰Kåþï?=ÛÐ9>0?Xíg²ÐÒ?=ÛÐ9>0?ïö'Éüì?Q•ˆ¹®»?Søú/¤?Q•ˆ¹®»?ïÙá>/ æ?rŸ™Àk0?s`ÿøÙ?rŸ™Àk0?ï ý¯ r?‹Lo¾Ušú?Œ7ÀX«ƒ?‹Lo¾Ušú?ïÊäjMPÁ?d­vNpè?zÊÏ˲?d­vNpèAGN4FGL J1503.3+1651¿æòƝ¢Ž@Lï9C¬ÅÀ;4<ËbÀ<šáìÂo@ îÐ,Ӟ@Ü¢Ûa»?œ{á¢ÇÁ¿¢Ø€'y©?âU/<-­¸@³ch…$˜?ïÜe@Ìxê¿éÈLŸëÃ2¿æõ=Ïng½¿æ±Ï»"–%?ÁuîÚÛz¿âp· gAGNbllNVSS J150316+165116?ïø"1"m?Dƒ¶@p{?M³ÇwDãü?Dƒ¶@p{?ïõþ½ñÎË?Wˆ1|û¯^?T"cÚI}?Wˆ1|û¯^?ïό<0TS?{·àƒBR&?x9áõ"Fg?{·àƒBR&?ïöâ¼gÍ?AºW·VŠ?R:‡XVÓ?AºW·VŠ?ïíθñ^ä?aâ£[?b1GSYKÿ?aâ£[?ïÁ  ~?‡…#™?o÷Šȟ?‡…#™?ï»Ôڄ¾?'gÀg\?9ÊÊf²'?'gÀg\?ï¸?²¦
¤?y±ãYW'j?ðY"=?y±ãYW'jAGN4FGL J1503.5+4759?çý!:Q#@Lx•¿ðExÀ9²amaÚÀ<I핚0˜@ÜB4-@"j㣨ç?²âÚÖ$å=? Èé_Ìæš?ï
	žs`@	4\Ç×­¿áÛÆ«±Ê¿ßێ0¯Ë4¿ä?KâCW¿âyÃ:|Ô¿çhƒweR¿à"¯\y}šAGNbll3FGL J1503.7+4759TXS 1501+481?ïþ7ª€
–?~ښf÷?,…VN!yö?~ښf÷?ïõù/Æ!?UÞYPw?T
ŸíE9?UÞYPw?ïõí÷?`ÑrE9¢?T%Å´šø?`ÑrE9¢?ïäA°EúØ?XyM7¬û?k¾O´…Ç—?XyM7¬û?ïû
lx?9Œ8=0æ ?CÖPRáR¸?9Œ8=0æ ?ïØmYÊ¡¤?tæG^A¶z?sÉS8;Ѭ?tæG^A¶z?ïóâsä9Œ?b͓GK=H?X;¢À·#?b͓GK=H?ï£ñxös?x
«ÐÚù¸?‡¡¸0h?x
«ÐÚù¸AGN4FGL J1503.6-6427¿èI‡‹ÉDÀ"{¦iŒÀ9‡B,Ë:&À;w›9¬Éø@äuÚ͖v@¹NþjԊ?ÀÓbDé?ÁŽe³ãó@
žá×öÌ@
¢¸ý0?ïêž‹¥»?ĶúÓpTý¿é°Oô4ã¿â1i.—ÿïøÛH"?ÛmNâçxAGNbcu3FGL J1503.7-6426AT20G J150350-642539?ïùWâ6Ó?F¼êÖå?J wH÷æÝ?F¼êÖå?ïèz5eV?tf§ˆ~kü?g…éÍZYœ?tf§ˆ~kü?ï_¾P½æ?‹I]ÑsMö?"=ÙWß5?‹I]ÑsMö?ïö'Dà§?=g©RæT"?Rûvj¬Òu?=g©RæT"?ï¾óoÆ-ï?…Òѧ/·Ü?€C$å`c?…Òѧ/·Ü?ï^oÙEšÙ?©uÐöo/?"2×L¤ì?©uÐöo/?í§7Aé7?¦ÏN+c{?²ÆE¸?¦ÏN+c{?ï̕»¤Â~?hÞçÌÃj¶?yµ"3!?hÞçÌÃj¶AGN4FGL J1503.7-1540¿Ñ
)€E8@B?ÿñÀ9GúËã˜ÁÀ;Þª; g@ ~fpâ–?üLû[V?°ˆà <ó?«ƒÛÂ3?þÓðÈT˜@P†èçày?ïáŸØwü¿¼†ˆb¾¿àÐ^¼>¿ÓÙÔ½\¿Ýt§¼òå¿Öyɺɕ
AGNbll3FGL J1503.7-1540RBS 1457?ïûß}³ù?4©ˆÄœ?@'¾Í~ ?4©ˆÄœ?ïç¹
|?lß÷˜›¡j?hçFýË£?lß÷˜›¡j?ïî:B:ô?cs0RÈï±?aÅüš	?cs0RÈï±?ïÎڟ"{a?ahyënB'?x'°Cñ›µ?ahyënB'?ïòÉtŽÙ]?TZ7œ·ûÁ?Zm´æ?TZ7œ·ûÁ?ﮝ\û6J?Š³
ç|Ùù?"X¨¾Çr?Š³
ç|Ùù?ïÛâ¶F'?x"ÎïaVB?rü)¬*Ò?x"ÎïaVB?ïh3Åv¹'?€ˆ*ð'Nu?'ù‡Rà›¸?€ˆ*ð'NuAGN4FGL J1503.7-5801?èZOׯ?ݦ‹D—3¹À8%ª]6;üÀ:Dã¼ÓZ†@BÞS\ôM@ÔxþŸ3?³ ~Ôá?ÒL''ØÛ@!€¿®Y?ïî‰ÿó–?íœtà|¬ú¿š¿?#49¿ã§ÿT0¿è%d=—:D¿ëê¹FÞ
ã¿éý¿è,AGNbcu3FGL J1503.5-5801WISE J150334.23-580119.2?‰ÞS'6>z?›'®T!üe?±àbV?›'®T!üe?´`:£üY?±,±ážr?ísø«€u?±,±ážr?ÂZil´?­ò('ê?ëiz»e¤Ó?­ò('ê?œ<£ÊJš?'È.Ì«ó™?ïáh÷L?'È.Ì«ó™?"5³Ü?³$ów?Ù?ï¯+‡ÿN?³$ów?Ù?ÇŸ†TÛ?"±‹^àŽŠ?ï¸ã½Ãß,?"±‹^àŽŠ?‰¥`ˆg(i?}¾îrxë<?ï™j}Þc^?}¾îrxë<?>sGu¥Ûú?1†¥Ãæ?ïü1–ûځ?1†¥ÃæPSR4FGL J1503.9-4247?ê"!…FÑ@+k{[À:5âÏòÀ;ý+ÐhbÀ@‡[ÿZ>@O¡—Zû?ȅ#ÖH÷k?Ô©Äõgö‰@^n<ô}@ITݧæ¿ïÿýFKê?ïÿÞý¦ßR¿å€èÈ«ÕÜ¿è>¸c­O¿ïþ³íQ¿îv¹?|AÅAGNbcuPMN J1504-4248?í÷X㵶J?±I2ØÀ,?°E8âÀA3?±I2ØÀ,?ìðuÞÔaA?·Wå$g?¸|Q
¦Ðx?·Wå$g?쉞¸£†>?¤¶ÉPý"·?»³
:ãÎ?¤¶ÉPý"·?¤Pµ?¿E0ÓàÒ?®–'*¦?¿E0ÓàÒ?é¼Q|ÊUú?Ãâ´ ÐÒ?ɺÖ¨?Ãâ´ ÐÒ?àµ*Ø>?Ò¼ÁË֜s?Þĕ«ÎO"?Ò¼ÁË֜s?ã
ñØõÏû?¹¢«¦Œq=?ÙêN`	?¹¢«¦Œq=?â‡Åµ?½©ý®°ÆÌ?ÛÀñüuö–?½©ý®°ÆÌAGN4FGL J1504.4+1029?Øb˜)_¨@KJ¥ß"9çÀ6Uü6GÀ:ð·E|@á9Q/r‰@þÆDƒ?€OH¬[?¹>àæ_E
@1`m?ž{@#MG0– ¿ÅiÌLtM¿ßzûÿjXä¿ämÂæ™ým¿ägHÐöR¿é:®ƒ¿ëŠ7KšAGNFSRQ3FGL J1504.4+1029PKS 1502+106?ïàåKQj´?iÞ¥3)?o´ڛä?iÞ¥3)?æa÷/»ž@?Ñ´õ U p?Ó< ˆÃ€?Ñ´õ U p?îN"͵U?¢yÁ¤ãj?«Ó'>d=?¢yÁ¤ãj?îc"›%¥?»jØC¬ß?©Ç¾Xs´?»jØC¬ß?ïËÆ+ÀE?v•Åøeãz?zq
l1ƒ?v•Åøeãz?ÕSPW?Õ%ÔUWJj?åVt×Ôxú?Õ%ÔUWJj?ïFÕL«²Ô?•T}Y×?—%Vo±m?•T}Y×?àÐ^‰%?ÎçYòJñÒ?Þ_Bíݵö?ÎçYòJñÒMIXED4FGL J1504.9+2027¿íEeh ¹…@Miáâއ	À:'èYñ
À<q¾7Ô
@•)h¯@¼l}ܟ?º8yÄ<¿£Š~•?åtU!š"{@ñm@U¿æ°,X¿ã8Zðž´¿çu\}ÚKf¿áÕë#Ïèá¿ãކžR¿ïÝ€ÙYAGNbcuNVSS J150503+202811?ïô8Å0?Oï~XJv¨?WŽÃÿ«È?Oï~XJv¨?ïò¨u÷ËK?f
ôÁOÄx?Z¯)&šÂ?f
ôÁOÄx?ïØoö»'D?rÞ(¸-Ÿö?sÈ 'š$?rÞ(¸-Ÿö?ïÞPÝ̈́?Wƒ†³¿?p×ûïmT?Wƒ†³¿?ïÌÆ3ÍÚ5?pàTVñ?yœær½M?pàTVñ?ïù¨­³­?ˆ…•ð¸Q?~#+–˜E¤?ˆ…•ð¸Q?ï–M¥,þC?ŠÑçaû'?Šl–¸0?ŠÑçaû'?ï,;mûlY?‡°8ï2X?šx'E¹Þä?‡°8ï2XAGN4FGL J1505.0-3433?ݕkQ‡²@4°•9¸ˆrÀ: ¤¸±À<;2U½¡·@"¨¢J˜@…êZ|MX?À3ˆX(¶?À êæ`G@<9ҍ×@
†AÏß?Þé;'¦†?ïâӟNå@¿ä~IÏÞ¥¿âX»¸¨Rš¿ç
z!¯'J¿ïÿœb¡µÈAGNbll3FGL J1505.0-3432PMN J1505-3432?ïüñ³?Lށû½žs??/棂%û?Lށû½žs?ïãâßÍtV?u*èú"y+?l 	PYá?u*èú"y+?ïé³;Åí¤?h'ÀCg`?fLÄ:[³?h'ÀCg`?ïð4ô‡?EᑤG?_–é¹µ?EᑤG?ïòºIV?W½ÐÿŽ{?[ÅÀ›ësK?W½ÐÿŽ{?ïg@ªP\J?Ÿò±¬Ã"€?"ê»à¶?Ÿò±¬Ã"€?ï©?‹¤?ˆeÓÐih?…°±Þ§?ˆeÓÐih?ïʇ•¶
>?jµ»…^ê?z¼56(í?jµ»…^êAGN4FGL J1505.0+0326¿ãÐù=@I!lœ
"À8Ó§óÏpÀ;ìнU¡@;Ò2¸@ê¬azŠ?©ˆa97??¹^èî–v$@`dÄ¥¶Þ@/½É¤¤:¿Ð"h<ªUT¿ãµ´ÂêÌ¿è1¤½º
R¿èšc"åV¿éœ¦š3¿ïÿrܖnlAGNNLSY13FGL J1505.1+0326PKS 1502+036?ïøN饩%?_ôkGÜÃ|?NÄZ-ñ^?_ôkGÜÃ|?ïñ‹<M|ú?fä@P7?\é†á6?fä@P7?ïeDWȾË?':Ÿ€f×J?"Wu
W–?':Ÿ€f×J?ïà_Á†"?]øê/.Ò?o >L"Æ?]øê/.Ò?ïø,¡kœ?Rá×/ƒ#¬?OMz–*Í\?Rá×/ƒ#¬?ï|ÚBùq=?¡wNQWò–?d·Ÿ
c?¡wNQWò–?ïR±^?'`kÎÐË?•©Ô7?Ö[?'`kÎÐË?ï}LÕ×ɑ?ų=°•Ú?VeEÍØ?ų=°•ÚAGN4FGL J1505.5-8241?éÆO?Ù4À4ú9櫛$À:¡Ñ'¥`wÀ<}kgW'.@ >K¶··'?ÿ¤;~[O²?Âsýiw¾?©/†DA\?é«ù®ro@ïÒÇÄ?Ä4<»Ív?Ë*ž¤›U[¿Ó=Ž >¹Ï¿äXý'«Æ¿Ó˜úìð¯¿ä*[…~AGNbcu3FGL J1504.5-8242WISEA J150525.41-824231.1?ïü_uö4?2-zÕàõ*?=Pƒ¯ø?2-zÕàõ*?ïóó|äØ?\þSVú?Xü–ƒƒ?\þSVú?ïà®(ûT}?wÒÎi]?oQÖÁS+%?wÒÎi]?ï÷Dtq?6‰¡Œ@$Ø?QwñEØrb?6‰¡Œ@$Ø?ïö™jÛÒ4?K	‰®E_?RÍ*MÚ÷?K	‰®E_?ïÑK#êÀÔ?'>t0[Ãò?wZn!M?'>t0[Ãò?ïۋÏV"â?~CËs;Ð?r:uâÁ?~CËs;Ð?ïàLòˆ.?_/¥ÙU3?oý²æü1Â?_/¥ÙU3AGN4FGL J1506.1+3731?غ"µj@Mó'=[«"À8nd"ÕÀ<3mÖQ@D`%Z@/Þ|·â?Ÿ'†yù—?ºA–{@GՁ§4@Ÿ¶'³y¿§¯Þ™AÊ¿ãÑél?Ä;¿çO'ðßь¿ç¤8#\üZ¿ë=8À:î¿ïþ½	á*RAGNfsrq3FGL J1506.1+3728B2 1504+37?ïð	¿`Ax?hÌ]¢°·?_ìRºßÓ?hÌ]¢°·?ïñ¢bH¨?dÒZB?\»;Š,¯°?dÒZB?	°??‡;üWi
?‡•ý¥)<1?‡;üWi
?ïþ"´'ds?Å
]â?&ļJݧ?Å
]â?ïõlöoÕÈ?NE?H?U&—?¡?NE?H?ïЙö`Äç?ƒ›Î1Ž´?w³Æ®¥?ƒ›Î1Ž´?ïÆÂuS?"eôÒ(š?|žÿ1hu½?"eôÒ(š?ïüNX—`?1k'™'Tœ?<Á"µ?1k'™'TœAGN4FGL J1506.4-0540?á\˜o"!¾@Eܺ`À;{kà"êçÀ<ž`·Ð¼@"ìr'9Õº?øYÙû‰xº?×\ýç!?Ë©=¦~¯?ñÉa=1¹¶@/ªÁŠ$¿ï')` §¿ïéMcÓ?ï÷3¨£ø˜¿×§amÙ!o¿Ç<ú\Rn¿Ó^U`Y±øAGNbllNVSS J150637-054006?ïý|0ì˵?*q"³ö?4z‹¶…¬?*q"³ö?ïð\ºÒ4§?c™'dæ#?_F‰×¥²ó?c™'dæ#?ïDžwù‹È?€óYGª?|=D7œ?€óYGª?ïú'—õT«?=å%YÐ?EõŸ"@R?=å%YÐ?ïþ§'\Þu?%û6ÜþЭ?%‡Ýð}?%û6ÜþЭ?ïLj"b?€¤å:"?|;ð¬0??€¤å:"?ï͉$£Åº?ò²ûm†°?y;mÆÚRó?ò²ûm†°?ïð0-‰ÿ?[X'l'n?_Ÿ¥	Tá…?[X'l'nAGN4FGL J1506.4+4331¿éøxÞI]@M!ý`éNäÀ;CEћh§À<˜&B‰èL@xU'¾·@¶ŽYÊv±?ÃٙycCF¿§‡¾د?äöóaŒ@ö^KdØG¿Éà ¢6÷?îÁÿiW2¿âg`âC±¿å‹	H~¿â3''d3¿Ü™špY.oAGNbll3FGL J1506.3+4332NVSS J150617+433413?ïü\&Çj?1µ¯ÂxŸÂ?=È¿'…?1µ¯ÂxŸÂ?ïó¸x?^Ù8ƒ
Âà?YÓËÇNÀ¦?^Ù8ƒ
Âà?ï܌‹œ´_?u©-±9…?q¹ºQB8o?u©-±9…?ïèø[4ÈÎ?O
æ´w(_?g¤£[¹ã?O
æ´w(_?ïíG	°G?aœ³Xø3Â?b¸æ9¨Ú?aœ³Xø3Â?ïͤÀ'ç?z:ÄæS?y- ùP??z:ÄæS?︻ÈúÊ?'ñõðÄc?Ñ='?'ñõðÄc?ïlG¸°É?'ˆ<zÒ?'w	±PË?'ˆ<zÒAGN4FGL J1506.6+0813¿èvKŠ±¹@Jl÷ µíÀ9_N"¢Â7À;ÍßgDX@¯T§¢ò?ùŽ%)/?³¥µ%ç?¼<©>'X	@—ƒ>äA^@Û¯fœA¿Ü]ÝÙ¥¿¿…	ꏀf¿ÓþuÜ{ ¿Ô!}Uì¿Ý²ú"¯tÍ¿ÜÞì>Ø
AGNbll3FGL J1506.6+0811PMN J1506+0814?ïüçëYf?20v²kS?8Ço$Þ3?20v²kS?ïëf<8Ú+?uk†ÂϤ?d™ÃÛÃ|ð?uk†ÂϤ?ïÀËÉ[lý?Va(¡?šCÛ%›?Va(¡?ïÛÙÙøs?Rþµ&6ÑE?r}Ó:`?Rþµ&6ÑE?ïùZ¥Ï=?E©n=hGê?J•i)à9?E©n=hGê?ï‹o–!%P?™­1¯ƒ?$ˆä·ò?™­1¯ƒ?ïÄDy<èû?"O8?i#é?}ÝÃr¹ŽŠ?"O8?i#é?ï^]¿‰ÿ?t
%èXÙµ?Œ(h‰>H3?t
%èXÙµAGN4FGL J1507.2+1721¿æ½«Oà¤+@L™£!h0À:‰\qÀ<Wκã–=@ em¿öûu?ø‰Þ¦$ ?Ä/g Ë}?Îæ|¡;N‹@¹A|¢@	ت•yµ¿ï~Å`?ïp?}ÄPý¿©×!~CÁ¿×ŸlAqºW¿Ò`½§?õ¿ç"T¼÷AGNbll3FGL J1507.4+1725NVSS J150716+172103?ïö;áá¬?J@ì§6Ê?Sˆ;è¬Xæ?J@ì§6Ê?ïç÷9»k?sçƒBN]ù?h€£è}?sçƒBN]ù??å"?…B*AÓý?Š\00+T?…B*AÓý?ïÚ#TT&?\ðç)^Žý?röîi¼¹?\ðç)^Žý?ïéì]@"?eÅf‡ú?fðÙ¹°?eÅf‡ú?ï~o%kŽ2?¦"(óäõ«?2RŽ9¶?¦"(óäõ«?ïyÙ¤\?•B~z\2?ÐÄÎݐm?•B~z\2?ïƒ!-ÞE×?9ûÃ=(–?7´z°F?9ûÃ=(–AGN4FGL J1507.3-3710¿àçTñQš@25ƒƒ­Ÿ
À:_'j@À<L$s|Ï^@̤.Èë@wÖޞ†h?ÂXê§Ôó?ÁG֘Óv	?ýœ¹ßŠ?@W?Ñ&MÈ¿ïÉU^?±?íf.¢<Ö¿è]œ"I¿ÚébÖ#c¿ä%ßøù{'¿ïÿï¿@PAGNbcu3FGL J1507.6-3710NVSS J150720-370903?ïø¨h??C=0pE~ö?M‹ ê_iÉ?C=0pE~ö?ïáW"o?Âʗϊ?ˆ‡¼7ÙT'?Âʗϊ?ïßÿ÷òjk?k"¢gQ%•?péî'?k"¢gQ%•?ïÀÈÕqa?aà›Ñy?›•CßØâ?aà›Ñy?ïÈ¢¸žŽî?xe'ÉÈ\?{®£ºWpÔ?xe'ÉÈ\?í %nq?¼^ô&«³?²þԐ¶R)?¼^ô&«³?ïivwfÏÿ?'Äö+ú|?'Ñ1n2%?'Äö+ú|?î4¼óïY?š0"Ï|?¬´0ÂÂ<8?š0"Ï|AGN4FGL J1507.3+3341¿êÏú#G-@N·=CÀ;1@À<Ïâù^ü@  ¿þˆ1?ø¸¨RšÈ?Ó­Ü|m8è?Öõ·ý‡Õ¢@f݄ªõ@\[J©q¿ìiþ Õ®¿ïæ»@2u?ï›r·­¿×@>Æå,¿áp¿ïÿ⾦™\AGNbcu87GB 150531.0+334938?ïês¡beÑ?f¾ƒ•—"?eŒ^âR^á?f¾ƒ•—"?ïÔ¡ù ¦?mµ7µ?u¯("\?mµ7µ?ïsuZÊü¾?‰2Ü/Èý?''T¨X6=?‰2Ü/Èý?ïv"—»]?x=e¹Á¡?'/m
Wba?x=e¹Á¡?ïãS0 ÿ?l•qŽü¦?l¬Ï{T¶?l•qŽü¦?ï¤ò/TM×?›C"ά,?†Ãt.7?›C"ά,?ï=g0³œ?"Bbƒ¶a?˜SéœLŽ?"Bbƒ¶a?î¿f± /1?–7¥Ûí?¤	"íýõ?–7¥ÛíAGN4FGL J1508.4+7717?ätjžbç@B¬ÜY1ÊÀ:ò¦WíýŸÀ<ã™hò1á@c`í*»@,næg¨†?·ž¹¾þ$¿µÑž~ìÖ>?úáՍe®±@‹Í(<_¿ÔǙœž±±¿èï^¶¿â—À%çñ¿áž2OÞd¥¿áüE°ä9¿Ó9ïô8AGNbcuNVSS J150811+771819?ïþ½rå?<œúˆX?$.ir5"V?<œúˆX?ï÷R0ñ±Ö?SíKڔ?Q[ž\?SíKڔ?ïõãžñ?g~]"üÌr?T9ÖBÈÎ¥?g~]"üÌr?ïü½@Á«?ÛÁ2g?:…•úÎ?ÛÁ2g?ïü¦iê2?8)DO͓ë?:̯žÒ?8)DO͓ë?ïՂµ@Wù?yðtè¤_–?u>¥Rž?yðtè¤_–?ïì¼Á¼ÎR?u.9/Û»?cC>V6/?u.9/Û»?ïí×=F»?RžÑw»}6?bù(ô3¤¸?RžÑw»}6AGN4FGL J1508.5-4951¿åã~JïΖ@Ò´|lbÀ8´"}Ðæ7À;; 'oÿl@œY®ê@žÚH¶R?²5Iè‹o?Ō¨Å["P@sœcxu@–,ÞZi?Ø¢@\;•,¿æNI¿ê5`Iô¿éF3 ÁV!¿î 2:ïÿóÖ&ãAGNbcu3FGL J1508.7-4956PMN J1508-4953?ïÉÕí:‰?{º'-,U?{	{x¢ ?{º'-,U?ï>Óë$%Ï?˜Bq(\ ¯?˜%'¤L?˜Bq(\ ¯?îcLÇóñ?&tÝ`?©Ë3"6¼ó?&tÝ`?ï7uÆ?~]'êÂBé?™=¶Úî?~]'êÂBé?îƒáþQ?«GOUðÐÍ?§ÁàZÊ?«GOUðÐÍ?éS¼¦A¦F?ǜÖ"i"ø?ʱ
fùfç?ǜÖ"i"ø?ë7ÏÒvì?¯›²<l†«?Ã!ÀÀ¶$P?¯›²<l†«?ç_'ßP?¶÷±§ØL?ÑA±ðA_à?¶÷±§ØLAGN4FGL J1508.8+2708¿ï´š	/@MÄ6~ANÀ: $-ÿîÀ<Rv‰Ê@~ÄN##œ@¦M™æÆs?ºâL¤>Ó¿¢F—'×Ïú?èŽÙ·–Ú¢@5ù¥ž?ïìh ¤Ñ¿ÙãºÚ±çÄ¿åëÍ
dl'¿àSÞ9ۿׯ͸…,¿Ôá,Ö!à%AGNbll3FGL J1508.6+2709RBS 1467?ïõXûªìä?P¡SG0ÞH?UN‹é§?P¡SG0ÞH?ïñÏVŸÑ?d½Û
qs†?\aSE
Ê?d½Û
qs†?ïâ3ü(Qz?lŸt'éi?m̦4&?lŸt'éi?ïÎÐÊ!:§?\?FÆ—?x—šØµ@›?\?FÆ—?ïÝW D»h?hZÄ÷O‰?qToî kÈ?hZÄ÷O‰?ïÁ—"ɺ¸?ƒIÂïç™?46:¿¡?ƒIÂïç™?ïÔ+©Î?y
†&{d?uñꌧøë?y
†&{d?ïÄ¥$Öé?‰}»&8!O?ŸÇkY­Té?‰}»&8!OAGN4FGL J1509.6-4334?Ý'å—"@)Íl.ýDÀ:êHޖ#À;á•ÊØ@Èý4s¥@¡íý¬i?Ë|,Ñð"?à.Ò`Š"S@})Àµ@n埬ƒ?ï¥(xÅ
¼¿â¤9/Ìvf¿é½¿ÚËé¿é×ñ=Å]m¿ïÿù_|è3?ïg4ø/Q&AGNfsrq2FGL J1508.9-4342PMN J1509-4340?ꀩ'<?ÄK€‰ĉ?ÇýýY»ê?ÄK€‰ĉ?䥃g~?ÏB°ò¯="?Ö´ù1Øþ?ÏB°ò¯="?êÁÊ(
hÂ?ªðí&3Å?Äø×_Ö\÷?ªðí&3Å?ëÓ_}éå·?¥<]êR*?À²'Xi#?¥<]êR*?ÜtLÁWV\?Ïk"":Æ6?áÅٟTTÒ?Ïk"":Æ6?³ãˆ++S ?À)•|ËÏï?탎úяL?À)•|ËÏï?ÕѬIce?º¶z-¡+'?år—)ÛNM?º¶z-¡+'?Åùî\Ù9?´	fÐ`f?꾁"hɲ?´	fÐ`fMIXED4FGL J1509.7+5556¿çÆÔ\°|@Jo~=ÁÀ:@K!JÓÀ<ŽævÁþ=@ 0@	‹€?û÷.?½iSWjö?ÀD,?Nœ@Z'£S&?üöèˆ?)?î0Sà&ñ±¿æ·'I%E¿Ý2;;•Wk¿Ñ¸䓒ï¿àñ¥"yŸ(¿ë'ž^ÿëAGNbll3FGL J1509.7+5556SBS 1508+561?ïùÐf'ä§?C3̾½ž?H¾e:îfé?C3̾½ž?¸üWÌ?ˆC‰ðîºê?ˆ[Ë8àã?ˆC‰ðîºê?ïßírׁ?s(áH¨?p	F—=o´?s(áH¨?îP.¼´"_?Šî¡ÝM?ªý6oˆ?Šî¡ÝM?ïÑÝ Y§;?s̈́ódO,?w/Ðl²b?s̈́ódO,?îUB@†?·À¥…IÑ;?®J«Û·D?·À¥…IÑ;?ï'JÞ© Ô?Íµ0~?‹­HKh÷?Íµ0~?é¦emJ¹À?«Ý5—ïE?ÉfjJÕÿ?«Ý5—ïEAGN4FGL J1509.8-2906¿ïÏ_·
¸@8¹yŠ˜À9'[4<ËÀ;ùÙLJ®@Rü'G—@3n<½€?¸'Þ½?ÁÇp×ÙpI@Š.oKè@®w!I§¿¨ëÂlÕ¿çòÖKÒ¿é0]€c½•¿èœPbîâ¡¿ía¬ÃB
¿ïö¾7ޓŸAGNbcuAT20G J150945-290502?ïùµ•šþÁ?Bp–ÚR¯Þ?I)©(Ñ- ?Bp–ÚR¯Þ?ïë"8ðrª?u€øÎ1v?d{Ç-}"?u€øÎ1v?ïÐj°3J?rv†Ytà-?wñJ¥&ªä?rv†Ytà-?ïõÝ´ùG?@?5ûˆ™?TD—Gþq?@?5ûˆ™?ïç+ŸãW?gŒ¡g±þŠ?hÔ_çù?gŒ¡g±þŠ?ïšYf3÷º?™±ÿ5£¾?‰i¦l"Ùm?™±ÿ5£¾?ï=ãSÿ˜?'¢s>r‹?˜Cœ'q?'¢s>r‹?ïÖñQD?mA~lmï£?~4‡M¿	?mA~lmï£AGN4FGL J1510.1+5702?àÕt@IªB¿˜0äÀ:¢<g[RÀ<ª4òP@¸ˆå—I@
4˜?½€žöЬU?fmȁúƤ?¨á߯\Ï@ú8õêÓ?å4ªÌÇÄO¿çvÇý°Ž¿ìܽ¹‰y¿å/hۋ¬¿än,Rn¿ïúÎg×®AGNfsrqGB 1508+5714?ïó¶Èu+?fd<`'6?X'oïR9?fd<`'6?ï÷hê
†?V8ë1Óhô?Qß.)+C
?V8ë1Óhô?ï©‹09?‰ßٔ½Y?…¹:ÐðÐ?‰ßٔ½Y?ïù'\8 ?4#£^S(ø?I·"^a†Ö?4#£^S(ø?ïñº»Zè?d`W~ÐK?\Šˆôù™6?d`W~ÐK?ïÝÜ(¬¾Ý?r¢P<ýc"?qëÀýé?r¢P<ýc"?﹘GèŽ?…zbò"…Ù?™îˆ&i?…zbò"…Ù?ïÛê$ݖ/?c"UŠÆ?r
í~§¦?c"UŠÆAGN4FGL J1510.8+7959¿î¶ª'í…@A•¥CñÇXÀ:ßB¶]õÀ<êž…@¿kÅöÅ@Eʯ¼Î?Â(Cg2ê?«
jØf?çù4j¤9@êÓ_Ž¿ç4yð'Î?ïî6¿Yǝ¿çD{û#!m¿Û§˜€|¿â«5£OûÁ¿ìïÐ!ëãAGNbcu3FGL J1512.3+80051RXS J151026.3+795946?ïÿ)Hx¿¯?í©žêÕ?Ö÷Vl?í©žêÕ?ï÷yÊ$ž?RazªÔG?Qk~?T`?RazªÔG?ïõr6Âù~?Vš3¨½
¾?U'íã!?Vš3¨½
¾?ïþü2Ð&?¼öx­­;? >PgûÆ?¼öx­­;?ïþû軍,?k™¼EÑç? Asó*"?k™¼EÑç?ïÙ÷ìúÙi?uƃ!}D?s	'§@?uƃ!}D?ïôðç֊Þ?dpጝíÇ?V0$/"(?dpጝíÇ?ïý÷H[?$]·£•Oï?0C–s¬'&?$]·£•OïAGN4FGL J1510.8-0542¿ÝLMn@Eyùa€M˜À8ؔqÌÀ;"
ɇï@["Ì´@71½è?©°åæyF=?¼¼"Ûw4•@YyámmÂ@P¡ú'+6?–ž=¿Ò¨˜Â¿åÇ#ªÿók¿ç;,%ø¸
¿ê¨¿;ê'Ú¿ãkÀx*´	AGNfsrq3FGL J1510.9-0542PKS 1508-05?ïúý—oó®??¥=[Cê?D	¡±ÎF
??¥=[Cê?ïßö¨Ææ·?}òæµ?p«­º°7?}òæµ?ïz…:"L?ŒB>cÉñ?¾/Zs"€?ŒB>cÉñ?ïٞžU?ZâF©V(í?s0°èâÍ?ZâF©V(í?ïöØG2?R¸LD¬?ROqæúÛá?R¸LD¬?ïÌŒ5-?›'ÆÇ­¼?ŒŒÝâÉÊ?›'ÆÇ­¼?î"5vPá'?Éæ¢è¡	?§¼¨šñæë?Éæ¢è¡	?ï$ûï¯P?†{1I…!k?›`œ RH?†{1I…!kAGN4FGL J1511.8-0513¿í¤u4='@E[|þX`À9‡ž ç×À;ò鳍a@ ‡øø#è'?þR@ßÄ V?¼FHcÆùÏ?¨ã^^°¦?íé"89,q@ŸâÈÇ߿Մ'!W¶¿è¥žTê= ¿æ\º:¿Ç᝿C!h¿áà¥â}8:¿Ú}çAB?–AGNbll3FGL J1511.8-0513NVSS J151148-051345?ïý†a;P?+}Ñi.×?3Ìù¢ïÄ?+}Ñi.×?ïíRia÷?l·E[¾¿†?bb­—ýá
?l·E[¾¿†?ïè½OœF?pa˜=§j
?gB±#ý¡Þ?pa˜=§j
?ïì€á‰>Ð?Pp€Ï7Ž?c€`?Pp€Ï7Ž?ïýJȯ‡?0‡¥·ìý?5¯h3²?0‡¥·ìý?＀ƒ•m²?‡UÔ¾uÖ?€ßß#"^?‡UÔ¾uÖ?ïߕŒn¸Å?yþ¥¹?د?p59ÒB…F?yþ¥¹?د?ï°ñB´Ø?uz¾Œi±?ƒÃ¯c ³ï?uz¾Œi±AGN4FGL J1512.1-2255?ÖWÄû>@=~"î9.À9ÎޑoÀ<!שŸ¡@ 	øF£'?ýü}ÿà?¹‡5híJ?³ŠJq=Yþ?ûmAfҜð?ü=aèRdQ¿ÜŸ9`ô·w¿Ô¿eÛüëy¿åtïËÕV¿Ó'vû	 :¿Ûî›ÿzt¿çǸƅŠïAGNbll3FGL J1512.2-22551RXS J151213.1-225515?ïù<Š}zˆ?EªV1¡ß‡?K
ÖNμ?EªV1¡ß‡?ïË·'=º?ž«2ƒ?z$xÊ´÷?ž«2ƒ?ïàÐi±ÁÑ?k-ÉO‰g?o/–t¹Îã?k-ÉO‰g?ïµíQžû{?g¨Iº{÷?'"«"yZ?g¨Iº{÷?ïíôlÎàM?Ués
^‰À?b"iyJU?Ués
^‰À?îÌ¢Àê?²£2Gñs?£3ÕáǦ_?²£2Gñs?ï´w-*|ù?ƒG"·&ø³?'â4­!±å?ƒG"·&ø³?îOSlŽ|?—^s‹?«
ψ[1>?—^s‹AGN4FGL J1512.2+4704¿ï6×<½J¤@L>}QÀ;6©ðÿ±üÀ<äæíàBË@.KAò¿@\Ôí,¿?ÑqD:íg?³#uÐ玚?ãŒf«/Ä@E<O'²¿àdy¡*]¿æˌ%<Ðk¿æ¦j±N¿ÔyK%BY¿àÐI ]¿ïÿç@ìYZAGNbcuB3 1510+472?ïþX—_œb?Íu 2hr?*vˆ =ö'?Íu 2hr?ïö1O@Ž?WnøÏhÂ9?SÛ…:Ô ?WnøÏhÂ9?ïõ¡ VÕ­?RpÛdáS?T¼¿ÃÔÆ?RpÛdáS?ïù5$hÙÍ?1C S¼F¹?K+nmY/?1C S¼F¹?ïÿ WÓ?ú{wd"¼?»ð'…\É?ú{wd"¼?ïÕYßM
¨?y<Îüu÷?uSD-ñ?y<Îüu÷?ïñq0]¯¢?gSY`œât?]Ÿ­Ú²?gSY`œât?ïäÖ§Ó)n?XÌ$×ýô?k)X#7©™?XÌ$×ýôAGN4FGL J1512.2+0202¿æOâiÓ>'@Gý›#ÝTÚÀ8Öu£KÜÀ;ɑÆf>@ÁX';§ ?ÿ~Ö|¨È?ªˆSöø'?Ä'q¤€¨@#'\´5ý@SOÄ +¿Ùw<!™X¿×Du»Cš¿àþ‹ Z›¿â¬×cÿƒÙ¿é']ýa?5¿év%@OvAGNfsrq3FGL J1512.2+0202PKS 1509+022?êé€c_?Äåÿ…©6?Ä[Íþrƒ£?Äåÿ…©6?è·Rè?ʆºaî»?ϛÅ"´_î?ʆºaî»?ëc…^àFb?«ÔV_Å?Âqê"~æv?«ÔV_Å?ꑬq§Q?©}PãHÑ?ŹN9b»ü?©}PãHÑ?äÚOí9e?Ê{ÔÞOgX?ÖKÿ`%6?Ê{ÔÞOgX?ÎyØ°8?Ñ>{y%¹V?èa¾	Óò?Ñ>{y%¹V?æúÎ%΁ê?¹R,¤w
ì?Ò
c´bü,?¹R,¤w
ì?ÒeSzj?´"€5\'¯?æÍs{ÖBË?´"€5\'¯MIXED4FGL J1512.8-0906?êí&=κ@DËÑ$JbÀ5˜A‰7KÇÀ:k' ÿT	@VP"&ë§@òa|ÚQ?ƒÍ#Ç?¬ƒÖAsE{@'ö«ÿÍ«@!`&	ÿËÄØâ"Äö¿â'\f2d¿æÉÁ/á¿åŲÍÈ¿è2­œ…Ý$¿æð _ñØAGNFSRQ3FGL J1512.8-0906PKS 1510-089?å¬Xõ©S»?Üþ¹	‡¤`?Ô§N­X‹?Üþ¹	‡¤`?ï¸ÝwûöA?K²Ìi§C?È¡üŠñ³?K²Ìi§C?î$ö½i¶?¡£#Y>?­°"+m²?¡£#Y>?ïèH´'[Ã?fŽÞâô`u?g·K"ƒtú?fŽÞâô`u?îQÐ÷B°î?¶°&¥"';?ªâðŠ#?¶°&¥"';?ソ5+þ?±µÔUàºÉ?Ÿ¨HÊ6?±µÔUàºÉ?îÏÚÖ6?žÿ&à@Qg?£rPäÐÎ?žÿ&à@Qg?îó¢ÿÉÏA?›Ò"è†ho? ÅÐÒ§ä?›Ò"è†hoAGN4FGL J1512.9-5639?ߐĀD€Z?ðg¡á^TÀ8Ç£è_ÐÀ:ùҍ.#@T͆=,@dÆS6?´Œ4қ?ÇSy9QÛ?@àþ}=C@ÂÌ«êª?ïÿp\‰n¿Ð
,"óŸõ¿ã¤"CÆÿ-¿ß.ß[Å£Ž¿çIú?KÅP¿é·}z"AGNbcu3FGL J1512.8-5639PMN J1512-5640?ïÍY>'8?yEøÝ¡Ü3?yS`Ð$p"?yEøÝ¡Ü3?ïÀTaJÿ?'}îb²?ÕÏpLÕ?'}îb²?îT"}½¨? Ëø?ÛüÚ?ª¶¸3CÁy? Ëø?ÛüÚ?ïõ6æq
´?B'À¹(Ô?U'3uږõ?B'À¹(Ô?ï̓qê܋?'¤<ŒÚº?y¶Gz?'¤<ŒÚº?í'ië?¿™tÁÚ?³–Ä°9<c?¿™tÁÚ?ìEÑÙ¯'Ü?©À`–•?½Ñq2ƒq?©À`–•?ïÍeÅÆb?i"5|c¨Ç?yMÿ'W?i"5|c¨ÇAGN4FGL J1513.2-7131?íg¸$búÀ'c"ÀÀ:´Ôˆ'ñÀ<Wi¯Çˆ@"y¦	>˜@š"ÛÍÐ?Ä<yX¦?ÎcÜwµ@	£1…´	‡@«	¼Ad¿Ð(³"í?ïþ'ö ¿ãotâ«}¿àhþ&,"¿éU¯"­¡Ž¿ïÿÊñ*z'AGNbcuPMN J1512-7131?ïê†×¨¦…?d[©øû£?ey(pªp?d[©øû£?ïð/¯^ìŽ?gÌ!Š(_?_ ¡jó˜?gÌ!Š(_?ï¡õà0E²?€º'»²?‡'‡í["?€º'»²?ïý:Å<¤e?"šn⺝ ?6)×ÙC¯ê?"šn⺝ ?ïÐïã—?wbÉ 4pÒ?wˆTË+?wbÉ 4pÒ?ïÅÇ#¯K?"ÍåTÓb?}~YŠ²a?"ÍåTÓb?ík~Éè•?¨² í?´¤	±,þÔ?¨² í?ï÷,ÿèû?CÖË©}é?Q§Ó|=
?CÖË©}éAGN4FGL J1513.4-3721?Ú '¹¨@1h²ú"¯uÀ:b寺À<O)1Q±£@"®ˆ"
¿@˜säÔ*?¿ÊgþÓw?­¼³Ïû«?ñÞ¦éä5?ûŸ5åÀ¿ïo.áêÁ*?ïì¢À‰Èk¿å»àì>'¿àð™Ã¿ÞËrÅz%¿àpÊ"M‡ÈAGNbcu3FGL J1513.3-37192MASS J15131867-3720114?ïûUI;:ò?7÷ÑÒÆQp?BªÜiy>?7÷ÑÒÆQp?ï¦üo8a?'úpn0?†@ä'°"É?'úpn0?ïëËvû"å?fíÚ҉¦8?d4ˆá!*æ?fíÚ҉¦8?ïÆjjþó?d,Yó6þû?|ÊÊޜî7?d,Yó6þû?ïðàõ©:?R¿þP‡×?^>Ü­Œã?R¿þP‡×?í§T¨×WÉ?¿7'^.+?²ÅZº8?¿7'^.+?ïá)ÆÖqD?tÏáòQUX?nÖ9'|@?tÏáòQUX?î}äB›l>?˜•'NGh?¨!»Ø
 ?˜•'NGhAGN4FGL J1513.4-0753?é<–OHxÑ@DuáC|V"À;bˆRIxðÀ<‡çQ³Pû@"/c¤• 8?û§+y*Ž?Ò=ðüVþ?±b;^zߚ?ßÈ*[sCD?ö-.vàÜú¿ëBĀx
~?ߧnƒì3D¿ç+m´Z濾9HËö¹¿ïê[ãU¥?ï²Ã×ZÅHAGNbllNVSS J151324-075450?ïýòVE?2*ˊtd?3xnÉI>?2*ˊtd?ïÁM^œ\[?ÚøV
?YP·Q2F?ÚøV
?ï}1»Ü1?†¥§Ë´¿}?YȆ1«ö?†¥§Ë´¿}?ïÈPnWv‰?ooíZÚ??{×Ⱥןi?ooíZÚ??ïÿ-ÓÞö?!†›åŒÊ?FNp¥B?!†›åŒÊ?î"{é
'ä?¶ìöv‡?¦ÈAp	hº?¶ìöv‡?ï¯ûR=±ß?…©mV'‰+?"+däÜe?…©mV'‰+?îVLk¤¤÷?£L•–r?ª›9BFš?£L•–rAGN4FGL J1513.4-3231¿¹O•[ÊÀ©@5r›ÏÔ¿
À9v)a"YÇÀ;¼GÜ7£Û@ÛQv?Lq@á#ôÑÏ?µÀÈ\¥?Á•T{ç@ Öoþ@û0$
 j¿×9Fr«G¿åSFÎñj;¿ä›Âhż7¿çè0Àè#¿é{'{;
¿ïÿû˜'2AGNfsrq3FGL J1513.5-3233PKS 1510-324?ïûAwg?=kÕÌÎ/S?BùùaÚý?=kÕÌÎ/S?ïçyÔàË?zVe½I!?h†+=q€Æ?zVe½I!?ïÔPÀû?o­Â!qÿ?uן"Õlˆ?o­Â!qÿ?ïþb˜È۞?€ÂÓkÍþ?)ÖuMCQÊ?€ÂÓkÍþ?ïì !sO?_§€ßÑÈÈ?c_ÞyªáJ?_§€ßÑÈÈ?ï`¼:ÙE?¤Çøêœre?"ýès}ml?¤Çøêœre?ï–.fV?"•¬ÔÃ?í:4í
-?"•¬ÔÃ?ïùM±p?>ª±sî?JɊ$þ™?>ª±sîAGN4FGL J1514.4-7719¿íu#2¥À0¥Ì·ÔDÀ;ǀ¾/À<àÔfõŸ@"á%T"l?ú)'jÑ/2?Ñ°Ëdlç	?Ħ–—±?ó¥@Ìxé÷@åÕÑ-Yª?ÉðXC=—¿ïÃh4œ¿¿?ïëÇkcü?ÛCå½´€ü¿îHFøã?獨eÓAGNbcu1RXS J151448.8-772249?ïù'ß —˜?F¯¹Ò#ÿ?K`'7ÿ¡0?F¯¹Ò#ÿ?ïñÖ¨
?\	rʖÊY?\SôBmu?\	rʖÊY?ï—<…þmj?€EåXZL?Š0ގ#o?€EåXZL?ïðýà"ÔT?UyRETð^?^>rfWØ?UyRETð^?ïøÎò°¥é?L$ñÔë?LÄ5Hg?L$ñÔë?ïÒÈ4Ë:?}¸F•ý*?v›åè<jñ?}¸F•ý*?ïRHTá?ˆR‹¸çYï?ˆ¿kgÇ?ˆR‹¸çYï?ïØ=gO֓?qÒÊ09?sáL@·^ˆ?qÒÊ09AGN4FGL J1514.6-2044¿ïÒ÷ޕÄo@>å.rÚ0À:uÜ£¥§À<Ný&g@ìF±ë@ ¿þˆ1?Ã)Wɱ?³Ÿ™/Ò?ñ*¸¾«¢@25¯O>?ïÿŒÝÉtS¿ÝÀÆCÆ©G¿á$gRõpZ¿ãšÍv?ø¿ä;_‡O:¿â"«äøêAGNbcuPMN J1514-2043?ïý˜"yí?%@|Y†Eâ?3;dt9³ä?%@|Y†Eâ?ïïÞpýÝÖ?c|AOÏK?`!ŽûBòg?c|AOÏK?ïò%ö£y±?\ûÑíQ^?[´Bڏ?\ûÑíQ^?ïö'8¸i?6î˜itp£?SÊÛÞFž?6î˜itp£?ïüð"‰º ?6b†÷ˆ­?8~êΕ®–?6b†÷ˆ­?ïÀhœ»Pè?".˜c"?˱²Õ«Ê?".˜c"?ïímÖ(Â?p/r:°W-?b')ÑNX?p/r:°W-?ïۑ۬…ý?\6hÎ	¶?r7GI¥n?\6hÎ	¶AGN4FGL J1514.7-3617?îuMÒpУ@2)•þÚfÀ9ñâ,°b3À<ßMØÐç@1gIp@e›Ã?…Q?¹ì6Ÿþ8?Ï›À:m9@;òá3Œ@©›''3?ïàÏ6iI¿ÝóæÐ_~¿ã9 ²ýï¿æTF›œS¿êjáj)¿ïûÊYêWAGNbcu3FGL J1514.8-3623PMN J1514-3617?ïïãõÁ?‹á"Úó#?"«È?‹á"Úó#?ï˜üF?ˆáÚå?~³ò:I4?ˆáÚå?ï­G©ëT?'÷ÓՍb??ž
W›+‡?'÷ÓՍb??ïÔ|ÁNj?X"µ<¸ò?uÁŸ
§k?X"µ<¸ò?ì·~^ª°B?³F:™',?ºD
ª}í?³F:™',?î@+ë ¨?¸'S
³?«ýNE™xs?¸'S
³?äô#®/þ ?¸.<îÇ?Ö¸£ ¿?¸.<îÇ?îçé;ÿpÊ?†Ø	Ð8+?¡l=u>a?†Ø	Ð8+AGN4FGL J1514.8-4748?íÑ]'ì³@ Ü˞Ïc€À8ñOäCá×À;y´{/P@ÔT¥sÂo@M/ãóYÿ?­á©þ–žh?º">eìC
@
~BZîc @xŽëád?Ýw€À政â,'à°«¿äS0¿äÕð'3¡m¿èÄ]'"ƒ¹¿ç ¿B Ž€AGNfsrq3FGL J1514.5-4750PMN J1514-4748?ïøù/Μ'?J+d#G5?L@]¨‰?J+d#G5?ïÓu-(­?ƒ
›8F?vEiO|¥z?ƒ
›8F?ïΔ›‹"Ò?w|œ@?xµ²$è??w|œ@?ïð/HJ¥?C–(ÓR?_¡o?%«?C–(ÓR?ïçÔ¨ÁÞ:?fJæ¿ýZƒ?h+WGŽa?fJæ¿ýZƒ?îXª@…×?²ø6ã¾l?ªu[õêÀb?²ø6ã¾l?ï-^TkŠ?"÷è´jó?ºT2òÔ?"÷è´jó?ﱍà'Ï?n^Ù®JiO?ƒœ‡à1¢?n^Ù®JiOAGN4FGL J1514.8-0949?è*ßã¼@C¢õ˜ñÀ8äŸM7ÁÀ;;Ò\XÆk@RgÈOƒ@aC?º"ÄÐÿâN?Ä?ðEwÙU@(»ÆKç@ƒá…Ói¿é¥Ï½—ûŠ¿äžæ.CŠ¿ã؎¡îÒ±¿ãÇÏ7
XI¿è˜Ï¤îar¿ê2ßP]¦AGNbcuPMN J1514-0948?ïúŽJŸÐ.?ERò?½â?EÆÕZÐcî?ERò?½â?ïò¼Vn1ó?`ÁÖ,OœÔ?Z‡S^J ?`ÁÖ,OœÔ?œýN?‡<¾-ióù?ˆÝXæ?r?‡<¾-ióù?ïÿeáò,?¢Ü×èyô?]B•È/$?¢Ü×èyô?ïßÒ»À?t'àoÈ	!?p¢UP"?t'àoÈ	!?ﶈm!k‹?•'«o®.i?']ä§~ór?•'«o®.i?íà8OQÍ?£•Iœ¹Ü?°ÿ>aX˜?£•Iœ¹Ü?ïþ}¬S/¨?$˜$¹)]?(%6óÛíˆ?$˜$¹)]AGN4FGL J1516.1+4351¿ïi.¤S@L?ނ׶5À:ÉOµò–À<iàš	+"@É´¨"²z?üO§r 0?àxïÕæQ?ægë×TL?ý`« ªšs@…çë·¹¿ë~ê÷Z?¿äöHñá¿áº cÏ¿èΦ´4P¿ïÿšêÒqQ?ïú6È)¨AGNbll87GB 151444.4+440102?ïøðvu'?rßqX80?O>dJ¸ê?rßqX80?ïôÉ)
?ZPÍj?Vm®þ+m?ZPÍj?î²q¼Û¾?"{)D†'?¤Øä.ԃï?"{)D†'?ïì¥áC4?U2g'vÒr?cZ(·Ë³?U2g'vÒr?ïöÎÂ+šI?aã?)?Rb{VTÎÎ?aã?)?ïÙR°øA?yäw'vxL?sVõÂPÓE?yäw'vxL?Þ@ü?œó™cj'Ù?§d¢!?¥8?œó™cj'Ù?ï¿8€"Ó?u2t^%??€;qéÑé5?u2t^%?AGN4FGL J1516.5+0015?Épxg^¢¼@G}$
=À:$í`Á
øÀ<6ðÊØÖÆ@ª4†O@ßöZdÐd?ÀFý•lŽI?²À´æ| b?ñ §". @ÄÓ6Hfv?ïÿÿÊPË¿ã»l‡è—.¿æ‡Í‰‹.¿êT
¾ÊÖ}¿è'vYùpš¿ïýHàÄ{pAGNrdgPKS 1514+00?ï(é.ñô¾?À£Ú¿m'~?šâÚQÌ<?À£Ú¿m'~?ïëšU¬/?q†Ü¡­Ä‡?dçefûyk?q†Ü¡­Ä‡?ï6AVÑ6Ù?–?LSèê?™7Õ,¸\ã?–?LSèê?ï›1'²Õ?qI.™@?‰3ºò£®Ã?qI.™@?ïÍr–cŠ?…¶Ò@}iO?yFµ	LZþ?…¶Ò@}iO?ï]¦]f&i?¢‰Ë|\ö:?"K4ZjÊ?¢‰Ë|\ö:?îـjÚ¥?š.{{fø?¢gùN
$?š.{{fø?îæŒïðœ?–"»G½y‹?®Á—4p'=?–"»G½y‹AGN4FGL J1516.8+2918?š7‰üGÙ@M©'Dé>À:Òwú øÀ<‡Ó*´ßp@ò_­Ád@¯œ'r^?¾` |È念Ëœ¡
ý?÷ÑÓíR~R@?¾VèD?ã	Ñäç¡¿ÝQò;_¿èÝ۝ ~¿âfÚ_\†ê¿ïátú}à?ïw¹_‡¤úAGNbllRGB J1516+293?ïø…·(d'?DxPÏi?Mé#¶ðt«?DxPÏi?ïñ,úI?c‹LÁè\?]¦ºïºÃ?c‹LÁè\?ﷂ¡–¤X?€ÿÔ-Œ?'W•ßl	?€ÿÔ-Œ?ïØüåï3?`(|%ãdú?sñ ö"?`(|%ãdú?ïá((éc?j
]×8Åö?n××#\5i?j
]×8Åö?ïŠÕmIo?•ûÊÜÊ«;?J¤´—Ü1?•ûÊÜÊ«;?g"
é?Š±]/°ò§?Wæl!?Š±]/°ò§?îj"BD?šnÁÉo'?©^&´œ?Á?šnÁÉo'AGN4FGL J1516.8+3651¿ïíh ÿ@Lñ¾ne8À;"ªLÀ<Ò6/fö@³B§'@
ª]6;ü?Ä˝bQý?·x°ëŶX?ì®Ö™íý@æ]êÁÕM?ÞU?bžÎ¿áåÓ)Þ ¿ÍU*˜ë¿êo¼árKL¿ßœ_Ý
\¥¿×¡CœŒéAGNbll3FGL J1516.7+3648MG2 J151646+3650?ïþö7ª;R?ÓQ©»]H? œ'ð*öŽ?ÓQ©»]H?ï÷êUÚä#?R¯'Éݬ^?P+Ten;¨?R¯'Éݬ^?ï쫅2?mg^ïÅ?cTzÛ²Pœ?mg^ïÅ?ïûØ¿…wµ?&:S¿ Á??@ƒàs?&:S¿ Á??ïþ%F.?+`z;té?.M²7©¼?+`z;té?ïÚ&P¥?}Lñˋær?rìØ–uq?}Lñˋær?ïé¬Ó¡ìé?sb·B<‰ ?fS,-ø2?sb·B<‰ ?ïôÆ1ìÐè?Cù~²6?Vs›¸j°œ?Cù~²6AGN4FGL J1516.9+1934¿ïK`Ô+:ì@Kð®Bž
BÀ:l3¹jðÀ<]úꉯ@HnÃ>Ú@WC³³÷?½êmœ™ì?oÌ]Ûþ?°¼0Gpó@q[$=÷Ý?ä³½œ®!¿×ö[üÕþû¿ëʝþ-B¿áâ™Ýâí¿âA&»×¿ïõ
8h&ZAGNbll3FGL J1516.9+1926PKS 1514+197?ïý''¸vK?1ŸÌT B-?6Ãj¨4%?1ŸÌT B-?ï÷…á3"¶?]d¢ù3
?Pô=àNtƒ?]d¢ù3
?ïÕjK‰||?s»X³þ#?uJÚ!$º?s»X³þ#?ïûÕ+,?*Ã)<n‹?@«R÷ˆ£q?*Ã)<n‹?ïñÏ¥&"?Z2)®\AÈ?\`¶#íé?Z2)®\AÈ?ïÕ#´Ýd?'îޕ°)¡?usnÃõ?'îޕ°)¡?ï˜uÒ6'?ˆø7C?9?‰â‹y;h?ˆø7C?9?ïñ«ÈŠÌ?MlšgÐ-?\¨nƒtHç?MlšgÐ-AGN4FGL J1517.0+2639¿îâÙøj›@LÒÂ&€IÀ:¦7åI›UÀ<éᰉ @fâæi«ë@ü¨"1¡?Àæ'w2?˜hͧpÐU?×ւN8ó@«Çæ2)¿çsø`îW¿ÙJzAå}ž¿èxDµ;·¿Øñ±ž6ó¿åTˆM@ûs¿ðAGNbcu3FGL J1517.0+2637SDSS J151702.59+263858.7?ïý"ÿ¼Æ?*Eð\ñ^?3X	D»?*Eð\ñ^?ï÷o`
+Ó?Wäm*åV½?Q!?îh
#?Wäm*åV½?ïî ò×?[œxçe\?aê_¿41+?[œxçe\?ï÷UGÁEì?7añõ=é?QUpã(—?7añõ=é?ïú÷¯›Ûá??‰ttõ'<?D!AÛá‡??‰ttõ'<?ïØM¥éøÆ?xfñ¶o?sÙ-!ä¶?xfñ¶o?ïߘÕ,v?v²-vr-ˆ?p3•x^ É?v²-vr-ˆ?ïàK?`æÁä"e?oâr¿zÕº?`æÁä"eAGN4FGL J1517.3+6630¿ïA &"+Ò@FZý›¡²À;BŸÿå(
À<ÏèYmZ@̘×ÒºM?ÿJBÉ©+Þ?ÙÚ €a?Úڐڮ6à@u4½vît@^ðù²?âÊ¡¿,ü
?ê{|½ë³m¿ãøÄL0Z¿ç·¡Aƒ­õ¿ïþÁU F¿ìÿ8?®ŠAGNbcu87GB 151628.7+663843?ïøÈØ?Jpj—NPƒ?Lܛñá%?Jpj—NPƒ?ïéêÚ©Ú/?h|~¼ch?f%"à5?h|~¼ch?ïPä/Ù¦>?…V+'P,?•ãzjG?…V+'P,?.ÓÊd?p"R±Aòº?ôD..ò?p"R±Aòº?ïùà´¾Á¥?HâÄÃ"©?H}-Êâë‰?HâÄÃ"©?ï¹Ú)+È[?ó‰"¸ˆà?‰u±FWR?ó‰"¸ˆà?ï¿ž‰Ù?"öNKHšý?žh=VöÒ?"öNKHšý?ÃJˉ?•.¼0;ià?§—CÌ/.q?•.¼0;iàAGN4FGL J1517.7-2422?Ç%…'‹€@;"ŸDÔEgÀ7o¡vݬïÀ;$óMj@ËBÎܜy@¢U°5½Q?")A9R©h?#59GÊD@À"<jêZ@eŸ±aâ?™—ÿ)‰¿ßGà~ÛRL¿âÛ­p3T¿à¾Q	¿¿äæ
`:Ó;¿à˜ÖšíWAGNbll3FGL J1517.6-2422AP Librae?ïýJÌæ?3ÄFª¾©‰?5©žyyÂ?3ÄFª¾©‰?ïï&9XD?n×5	¦`?`áّ
Ô^?n×5	¦`?ï³"ÕÿÊ?ˆ^ƒc«?ƒ7Jz½­j?ˆ^ƒc«?ïû@¢©Úý?6ìjsX?BýuEâú?6ìjsX?ïûㆀ?ß?:ÅB0ö"û?@qæø
™J?:ÅB0ö"û?ïª+µîíg?——sñᦛ?…uv†6i?——sñᦛ?ïÀ6Ff—?‡Jg?D݁?ä¿_Œd ?‡Jg?D݁?ïöØÕø?Kö*¬jK<?ROÀ¬î‰?Kö*¬jK<AGN4FGL J1517.7+6525¿Å§¬Ï"à@F²-VÀ9e§Vñ~À<-s?'½@ ®F#û³?û¹9±Êé?«þDZF?°ìȀ6ò@àäJ7\@	ãÔùl"?ïЬU^f¿Ôœˆ Þ¿á,V4¿û-¿Ððú¾øxÍ¿ØlD̸«¿á$¬ó±³AGNbll3FGL J1517.6+65241H 1515+660?ïþÊ;߁?5'ý9š?#\C&V?5'ý9š?ïò®Õ"Æ?ZðëgÓ?Z¢Tþ²ìˆ?ZðëgÓ?ïö8äM?B©^°Ôç€?SŽ6ì՛?B©^°Ôç€?ïÔà֟½?YH)³,e­?u÷%Þ-j?YH)³,e­?ïý禺5é?#XXS‰<­?0ÂÈÙw{õ?#XXS‰<­?ïӔB¨Ø7?{\%¹°·Ú?v5ÞÉ ˆG?{\%¹°·Ú?ïñµDK	?d²T÷ä2±?\•Ýlk.ë?d²T÷ä2±?Þ_?x8ݏGá?¾ÛٖE
?x8ݏGáAGN4FGL J1518.0-2731?éì©OUcñ@8ü*í"1À8×äŠX³öÀ;ÐÞô@ï_íüGd@E^ÿiØ?§¤yá1L˜?'ô;X¬Ñ?ê?Q"W6@©¹qPON¿"Òæí4v¿ÉŸ0²Os¿âVæáËâl¿Üýð;ø ¿ãRÄþ¢1ï¿Ý%[[ÕAGNbll3FGL J1518.0-2732TXS 1515-273?ïþ=r~«? *7H?,/Ö2][? *7H?ïð[~9?qÏȉ¬ö?_IëL2Á?qÏȉ¬ö?ïïéX7"?lñF#±Ó%?`ý½Åìˆ?lñF#±Ó%?ïþmsq-?uÛÞô- ?)(όiDÎ?uÛÞô- ?ïýÔ+?1ϝ#?'?7Y_⑌?1ϝ#?'?ïÆ÷9¡¦?ƒ‰íêšæ?|"c'Íä?ƒ‰íêšæ?ïóÉYƒF?h›4ŵÕ?XmN6?h›4ŵÕ?ïýç¿õ×f?-qH3&¦?0Âšï¥ ?-qH3&¦AGN4FGL J1518.4+0750¿Â}OƒmTº@Iãø¶À;¥Š6OGfÀ<϶4ÚÓ @!æ©ÎÅöD?øFc[ïêß?ჲ<'Î{?Ñ[Þ£ˆ?ø@¢òÞ¯M?ÿ8n±d¿ï«¨Å†‡n?Öo'nÚ©.?ïኔC"¿À"¢Êšî¿Æ%
€œ¬¿é5<ø®ÒçAGNbcuNVSS J151826+075219?ïñ+c'?^w*¦–0?]©9^kQO?^w*¦–0?ïß÷q¡?'^ÉD<?pGabKr?'^ÉD<?ïB‰sAý7?'ÈŠ?(?—®Ñ™x''?'ÈŠ?(?ïÁ"ÃÁ¶C?láÊp×?6Ö
j?láÊp×?ïé1h>?hµÎηv?fΗ²Î›Ç?hµÎηv?ïc(6ˆ…Ô?¥\ åŸHÞ?"šù7†K€?¥\ åŸHÞ?îÿÚ½j?™áS+F
î? T+üm?™áS+F
î?ï]øiïÄ?‰*'BaÂ?"@òÅw?‰*'BaÂAGN4FGL J1518.6+0614¿ê¥áÚ:@H¥Ç%ÃÞèÀ;NÉ&O"À<¤À²W&@!¶¿•×˜?û·Š*ÍB?È8uý³¦?")ê4;ÆÖ?ÑÁ߇Oj?ýÓ*U"¿ïðrXâð%?ïÿýfG³¿ä·K%˜?ý¿È¾ð€±a¿â›ëþì.½¿¶W¦Úõ¯oAGNrdgTXS 1516+064?ïü¨9Ås'?5Iinu…?:¾/ÆÒe?5Iinu…?ïíBž54À?lXD%#?b½b䇈?lXD%#?<­Â'Ú?'ù"Ë•'?€ØÔ5¶?'ù"Ë•'?ïÕnócö†?`h±!O ?uH†EÅ­,?`h±!O ?ïúë†?A_\Mõ?DEV¥
ê?A_\Mõ?ï\QքÜ?¢]Á¼£^ê?"uÜ,œh?¢]Á¼£^ê?ïÅ^n¡¸?'5Á'
öÕ?}PøEïsü?'5Á'
öÕ?ï9$'(?Œ`òð3?"?˜Ý»mºÿ¬?Œ`òð3?"AGN4FGL J1518.6+4044¿æ[k½#@Lp'À‡D,À:¢"O…yQÀ<¡ã¼Ó[@ *4~6çž?üÕnvÖ 3?½ãpþöÌ?¶Fçeç¢?ú£é~´;@èîݘÌë¿ïýI׺f™?ïúþ§°´¿ÆS&ƒ!ˆ¿ÜèV*¯3¿ßìÑ$o¿Ù<ƒÿS‡¼AGNbllGB6 J1518+4045?ïüò"õÑ1?-[ø§°®j?8kÙ»3¿Þ?-[ø§°®j?ïå¾õz?lkˆÊòá?jA
'"Ru?lkˆÊòá?ïí³;£'Œ?`üÄ:ÇÇ?bLÄhÍs?`üÄ:ÇÇ?™É{?nû7»[?ŠY¡$?nû7»[?ïñó)zD6?YÛ§›˜«?\¬Ñ¾#ì?YÛ§›˜«?ïŒíÍÈ? –J9øâ?ŒÄ¼»B? –J9øâ?ïãñ«mEm?rß5€M–Ù?lT·Ö[B?rß5€M–Ù?îk¡0F´?"'M!?©Eî[CÆÊ?"'M!AGN4FGL J1520.0-0905?Û¬N֘ö@CwÏÃøõÀ:ÌØU—À<W÷øʁ™@ Ú³€ ?ÿ'º¤ê?ÇX›w•7à?Šû«Uè?Å™bg(@«"ÚJŽÄ¿ïÐ/",z²?>·Ë´¿åÄCá× 
¿ØóY^@'7¿é§Û?×$¿'aAGNbcu1RXS J151959.7-090434?ïü6H€;>?;vÓû¿hÎ?>M¼íןD?;vÓû¿hÎ?ïëy³u7å?m/˜¹˜–?d†Le¬R¿?m/˜¹˜–?ïÎÄ93?wÙ¡Cw?xãXÃ?wÙ¡Cw?ïîÇ9v)Ž?LâÈ]æˆà?a8ÆΎ¡w?LâÈ]æˆà?ïø¯xËe;?MŽ½œH7Ú?MBރMJ?MŽ½œH7Ú?EkÂ?+ìi‹?‡n¼eh?+ìi‹?ﲛ»)X¶?"áIp1Lp?ƒY7¹–k?"áIp1Lp?ï¤ÚªRpÞ?zÖŽÎ?a?†ÉUd"¨?zÖŽÎ?aAGN4FGL J1520.4+5546¿åäÎd¯g@Ilë¯#À:‹F¦­~SÀ<ÇúȈšn@29¹µú@'DEª.<?ºªlЍ̇?¥1B#Ÿ?çͬ[==x@²çôE¿ç£¥€š¿Ü	»€Hj¿ä­ÂC±Ü¿àAöD•[F¿æ ß=Ù¿é§E‰w§AGNbll3FGL J1521.1+5543SDSS J152034.98+554256.9?ïúÈuF p?NbeрÎG?DÞ**Å'?NbeрÎG?ïôDuzÖ`?Z"è9˜²©?Ww†b@Ð?Z"è9˜²©?ïó°î8Ç?`œCó}'?Xž#ô&Z?`œCó}'?ïå?ªpª?R%A¾Ë\&?jÀVMÆ?R%A¾Ë\&?ïó﯌n?TÆç¢g{Á?X ¡)í¤ˆ?TÆç¢g{Á?ïÓ²ŸzQ?x^¢ˆµÝ?v&°5ïÓq?x^¢ˆµÝ?ïîÊð¡?qʶxFÀˆ?aôðô×9?qʶxFÀˆ?ïKô'?wK|Tã$ß?Œ-$,§u?wK|Tã$ßAGN4FGL J1520.5+4209?ïÿýÝQÞ@L÷< À:——sN¬5À<•B›†ä@]"s퍍@*½Bì?ÄûÆnäº?ÄúÒB¬?ùé˜dæ3¦@³ÖwñS?¿·ø·otØ¿è•*™1¿äö3kgW¿éÞá¢Fç¿è_Jþ«í¿ðAGNfsrq3FGL J1520.3+4209B3 1518+423?ïû® xM?9žSPò»?AE~XFÀ®?9žSPò»?ïöå)v,?Y˙?SÄ5¢ç•?Y˙?ïå)òº¯?\f™¶!?jÖ
hHhÏ?\f™¶!?ïû1ÜhmŸ?+¦v²i5z?C8Ž»2&?+¦v²i5z?ïóàû‹"·?Xlf&æŒ?X>	-®Â~?Xlf&æŒ?ïÝý«ß8Ø?tVà%o?q*/ÿü?tVà%o?ï"¨-‡?ŠNü'bBÀ?ŽùU÷f=?ŠNü'bBÀ?ïï[Ð`U*?Lô©´^Ú?`¤/c1¶?Lô©´^ÚAGN4FGL J1520.8-0348?ïýq—
âÌ@E@j]këáÀ9e¾¶‰"iÀ;ÇҝÇ%Ä@ ®ÏÑ?øÁi÷ë^ˆ?·5ëŸJÞ?Ȑ°|_!#@U¨¸ñ@zkði	.?ïéÐÒj›¿Ò±Ä}óË¿¿ÒƒÒ‡÷°¦¿Å"¨™Þ¿ßÞ¼¹YR'¿äܝàP7PAGNbll3FGL J1520.8-0348NVSS J152048-034850?¾½ô?§ÐGNÊȤ?§î‡S89Â?§ÐGNÊȤ?æm¿ª$à?Ìâ¤Z<â_?Ó$Þ«¶A?Ìâ¤Z<â_?ìŸ@«§õ8?¦–Ì5¨Ls?»ú¢ÀV>?¦–Ì5¨Ls?ìNeyèŠ? áÏÛÝÒ?»…ŒÔ0»¬? áÏÛÝÒ?éŠëceÕó?Å㽥Ηc?ÉÔRrh¨5?Å㽥Ηc?ÒÞŽyŽ?й+7ð?æù¸úC9?й+7ð?ëQg–'(6?­j-`?ºa¥·_'?­j-`?àˆ'¯z	9?»
œ µ?Þï°¡íŽ?»
œ µMIXED4FGL J1521.1+0421?å­8TQ³H@GÖbýüÁÀ;<-šlþÀ<'ÐÛOF@¼ú%6ñ?þÝR¦–_?Ó+-€@Ø?Óµàaª@¡B‡N@:à\̉±?ç(-í¤?ïÿáÍì¿ÚÞ;õy"A¿âÄ»á˜
ù¿à¦ºŒ¥¿ïÿ€éŸkkAGNrdgPKS B1518+045?ïíUk{?k:ìf jŒ?bªÿk²5?k:ìf jŒ?ïàNô¸f?y1'[Ö?:?o±«MÙÏ?y1'[Ö?:?ï#+{ƒÙê?"¹ø£"ì?›šÌôÊ?"¹ø£"ì?ï§N›n…ð?oãbЮ¨z?†,Y+=¼?oãbЮ¨z?ïõ!Ù«?aÝè°-†Ø?UÉùÇKjw?aÝè°-†Ø?îî«»žëØ?±8SÄÓM?¡DFB"?±8SÄÓM?ïO;¡í?'*^b?–œÂ^'?'*^b?î—ÿï §?›šÀ…øš4?¦€'ê'?›šÀ…øš4AGN4FGL J1521.8+4338¿è)Ž¡Ãߓ@KÊÒ¡øã¬À:HÚgÀºÀ<P·»*ä@'fuªÑû@DEÅ.î?ÀÐd[õP?³FþÌX´?îÑÕJIÐ@#ö½8ÿ¤1óÿ&øN¿æÌuúX S¿ëÎÊϜ‹¿é^ÑF¯ú¿ïþÔ¡­dR¿ïÿøãúAGNfsrq3FGL J1521.8+4340B3 1520+437?ïр26ÖM?®;ÑvÜ~'?w?æëtQ?®;ÑvÜ~'?ïóZ²À?]ÌÌh ?Y?YJ›«~à¼?]ÌÌh ?Y?ïÉ`Ó‡Û?~WNO×Y?{O¿"šª«?~WNO×Y?ïåË6}H3?VjÄÑvû?j4É®²Ìñ?VjÄÑvû?ïí àË1?he«í
…A?b÷ÞüضÃ?he«í
…A?ïÒôiHîÜ?xÀ¡
ö)ó?v…Ë=ûî?xÀ¡
ö)ó?ïÖ¾\`lì?z¯c½ºI?t ÑÌYî?z¯c½ºI?ïMvӛóç?"öIÓµ1?–Q%…¢K,?"öIÓµ1AGN4FGL J1522.1+3144?ïÙ0B	‡5@L'€uMÀ6¯ÐÈÚÐÀ;,âó¾ý@þH¸Uœj@õ¯¯…")?"}k,fˆ?²LDÀé§@&k9:´0õ@ ^œAk°¿Ð9wн¿â®L·2¿æŒï'zß¿æ»Ráú0ˆ¿éK·ž'QÒ¿ì]Ñó¹AGNfsrq3FGL J1522.1+3144B2 1520+31?ïæjçÕF?j°Ž—Íp?i•Ú-9Ê?j°Ž—Íp?ïÇ]"Åè?'·S}{aè?|Q6 Ì6?'·S}{aè?ïµEgúKq?‡O=Æ·P?'®¦"¤?‡O=Æ·P?ïÛNٓ?lѲ?rX" wÿt?lѲ?ïÜÞ˜{¦?k÷†S}–?qòR®¨¾?k÷†S}–?ï=ÈÈ0[?°ÊONǹ=?˜\ì!^œ?°ÊONǹ=?頻?‹R¦?‰MÙ·à?…ðýJ?‰MÙ·à?X靊? h½s
u?§"Šqf'Z? h½s
uAGN4FGL J1522.6-2730?îœ_΋'™@8fnü7£À8¯®çúÀ;"Ú")=@G'%\@·g2Ë?¦aPÒÖQ0?ÀBLUÄÍ@Ó:aû›@}*x#¨?ïJ?SÒåì¿Ý=E@¿áÆipÜáî¿âeÁ$øÞ¿égM·B÷Ì¿èŠS«x¿.AGNbll3FGL J1522.6-2730PKS 1519-273?ïðP[üÅ?VҔ…[:¹?__'
6Œ?VҔ…[:¹?ïɛagE?†éý?{2OQܟˆ?†éý?ïRfUþ?'J!mUFm?•¼³05Ö:?'J!mUFm?ïä5¬Š7&?U¸ßRàö?kÊS''qè?U¸ßRàö?ï"ʺdý?Šû‡Ja£?ŽÍQŠ"̉?Šû‡Ja£?îæDìÝÓ?±œ%ÁkÖÏ?¡›±-×K"?±œ%ÁkÖÏ?îF朊Bl?¡ËzYÔŸ?«'–9ïŽ8?¡ËzYÔŸ?ïwZ
¬TÌ?yeï$
ñó?'¾Juf?yeï$
ñóAGN4FGL J1523.2-3941?幞aªiö@,Ï9ó@ÔÜÀ:š
s÷H¡À<&« ,ZÒ@/b™'Y@¥D]'""?҇BlA?یo¤þ|@‡XÅÉ£@ÃNú#"?åg' Ö9]¿×9PC9e§¿á¸n¦¦ÈV¿é*è¬&d¿ïD‹ûbâ?ê,Î?=­‹AGNbcuPMN J1523-3936?ï'r46#º?¦N}­Ôæ?‹£rë—ÙŸ?¦N}­Ôæ?ï\j0—ÄÐ?ž/åGƒQx?"r¹íf?ž/åGƒQx?î1žÇgy?–¼!ࣹñ?¬æˆ²'n?–¼!ࣹñ?ï˜ÃÈíH?q&3ö¡ë?‰Ï
È)IÜ?q&3ö¡ë?ï>‡WÖ3?ž½;ˍQ?ø/œ?‰?ž½;ˍQ?éãÍaiŸ?Ç(iQc†?ÈsðÊzY…?Ç(iQc†?éÛ݌k;k?°_ˤ{n?Ȑ‰ÎST?°_ˤ{n?ëΊ@zr?¨ñ¢G§¯=?ÀÅÖþâ9?¨ñ¢G§¯=AGN4FGL J1523.2+0533¿íEU©Íà@GùÆøÀ;$1âÑÀ<Ô{¦j@ BE‡H´@3c¿Âù?ÅZÒ ãe?q4a†'»‡?¬·øX$Ú@ƒ&ûíKÈ?ﱋÈö~w¿çâ³¾ÞοäӅþÝD¿Ù­_H•p¿èQrÿ&`?ÁûÃ	€AGNbllNVSS J152312+053357?ïûó/ÚZ¡?;Øê†?@3@ºQjl?;Øê†?ïô@ï‰eD?_ç
¿b]?W~!sæ'L?_ç
¿b]?ïÚ¼òí¦j?zÂǎíÀ?r¡†¨É2ô?zÂǎíÀ?ïí+›©1?Fd°~3?bÔd‡Vœ?Fd°~3?ïôx̚½?X…W8
G?WÞHöî?X…W8
G?ï¬v'p?'èý'¹í?"âX™,?'èý'¹í?ïªxµ¯‹?‹Pá[Ù?…aÒ¡Û®þ?‹Pá[Ù?ﶿ5EÃ??p7Š?'P2ži\?p7ŠAGN4FGL J1524.8-5904?Ý1Pá`¿ýªôj ‡ÊÀ90êþ;·À;û¼¤`@ü†x)²V@¿:I§ê?ÀM^7?³Ï1VT'?òá+^R›®@=ÂKIU?ïqéQgÑ ¿äÜ-'€wŠ¿å'/ò?M¿à@RÖfª¿äÇnôªah¿íV ö…-AGNbcu3FGL J1525.2-5905PMN J1524-5903?ïüÚÌiÐ~?0¨@¸/¶ß?9)›F¥Pf?0¨@¸/¶ß?ïßÔx+¤?"˜Ã^!?pÃóµH?"˜Ã^!?ïÌԙõ´ø?*
 Ñ{?y•³VÏ?*
 Ñ{?ïãÚçÓÊ?Tn"¡R­?l€$÷/õ°?Tn"¡R­?ï÷««a?Meõ¡$D%?P¨©ëq?Meõ¡$D%?ïx+DÁ?ž
ñ~:¡?ýšš×y}?ž
ñ~:¡?gµŠ«?dêúÛ	?"fNc?dêúÛ	?ïyÆX
û?~¢Zã'?Ýg8n<'?~¢Zã'AGN4FGL J1526.1-0831¿ï·ôãí$Ü@C$Å~#òNÀ:d'>2j¶À<UW1?=-@ ÞÙꗎ?üèÀ˜áãµ?ÄÔ~\|W¿?ÈaZ8Ô%@2_¦XĽ@(jž"dÿ¿ïí¿‹›ª?ïøÒ¿€#¿ÙHÝòd¿Ø¸ƒ¿'¨¿ê Æê4¼ ¿Ã%I:±ÃAGNbll3FGL J1525.8-0834GALEXASC J152603.17-083146.0?ïú>ßÜŒ?G]YEu»?G€ùÍ?G]YEu»?ïß¿Àõ©?z2r]ˆxâ?p Ú$o?z2r]ˆxâ?ï¶ÙRTO?ëkÎ5Õ?'I¿¬|4?ëkÎ5Õ?ïÙ=
Ícv?\ôkï1¼"?saz±[‰?\ôkï1¼"?ïæôù'¦Ü?oà'ò´$L?i©rk·?oà'ò´$L?ïw.Z×?šW·V?'=l<×0?šW·V?íÕ+…aJÀ?¥ZÑÚ>)¥?±V£Ö­wý?¥ZÑÚ>)¥?ïVp¬‡ÕC?…niéHp—?•1êmM‰–?…niéHp—AGN4FGL J1526.7-1529¿íÂ)Þ!ß@@J#9ÀìÀ:¬ðéÇ´À<f]ú‡;@ |o»Ï¤n?þaÝ4ùÜÐ?ÆV©Zý?¼Ùz°m?öŠ"é9?ýÿrêg¹¿í$

[³?ï鯁7x¿ÐÀ¸âŠ#Z¿á},±8ò¿à	gB…œ¿âçsâOëÑAGNbcu2MASX J15264667-1530269?ïýÎÿÏP?.ØÍÄWmt?1ˆߨè©?.ØÍÄWmt?ïÐp(î?€É
Ü6&?wÇ뇒 û?€É
Ü6&?ïîq‰ýfÀ?YEÖÈ8'?aŽv9'ÿ¿?YEÖÈ8'?ï½ÀŠºt?f!Hƒéb?€Ýjk9"?f!Hƒéb?ïû—ËÃ?=6Ð}ÿÕô?A Ó8^Ø?=6Ð}ÿÕô?ïᶋ9Q?­+óôý?Ÿ£É0P£Þ?­+óôý?ïí"oìw?lm—a?bݐ>$Ÿ?lm—a?î˜Q®QM?"gÜÕzè¡?¦zå£81?"gÜÕzè¡AGN4FGL J1527.3+3117?æt¿K¸@Kò`ÐÕÀ: w!ŸŒùÀ;ù"GÁ`@Á¾V<"@;`äFf?Æ? fÒÇ俯ÈԀÜo"?à¡…÷%@÷§f‹Ð-?î†'_8u¿ëIé7'¾¿à§û\,Q¿ì#ã@Òٿłìƒ÷Eò¿ïÿ÷fÔJpAGNfsrqB2 1525+31?ïû$Ò®tX?FË´™G¦?Clµ`H+?FË´™G¦?ïö ?r~?Xû¦A,L
?R¿
E]¹?Xû¦A,L
?ï¿c€‹‰>?ðS
m?€'èÌ\b?ðS
m?ïûUÜÞñE?0¾KÉ7Ý?B¨Œ¤±{?0¾KÉ7Ý?ïìA™þCg?h´#«.®?c¾eõ^³?h´#«.®?ïØÛÅhÝ?~|J²årÆ?s'p¥‡?~|J²årÆ?ïgšÇʍ?'KÇ¡JX?"Œ 'vh?'KÇ¡JX?ïØ(/Éò'?l"
¡³)?sëèy?l"
¡³)AGN4FGL J1528.2-2905?î8שcñ@6d)¿*åÀ;(9Úí!À<Rӓk@ aOƒöÅ@ž¡%Š?Ç{¹ßµ1Ñ?"'Ë´êz?ÀBE_Z®w@kÈíºX?ïo×ÿ/öh¿ç¥8ž¬þÑ¿Ô܋ò)ô¿ç…L»Q¿Ï¿'ýs2Ó¿çV¯¤ÙšAGNbcu3FGL J1528.1-2904PMN J1528-2858?ïû`2'í?:_7m1‹?B6±·Üq?:_7m1‹?ïè–ì/?uûè"ëb?gi'Å¡H?uûè"ëb?ïèsªØÂ`?dáqƒ?gŒUÀÀ‰?dáqƒ?ïøNoÇ®?7R9®ð9?NÆAòhZ?7R9®ð9?ïø%O3³¥?H"'úΙ?OjÁu|?H"'úΙ?ï"Â?}'?"ŽæIÀj?ŠÏxiAcØ?"ŽæIÀj?ï㱡‰cR?rNŸ¸Q¥?lN^]ß~]?rNŸ¸Q¥?ï×D18?f/—1\[Ý?t]öþÁü?f/—1\[ÝAGN4FGL J1528.5-2240?± ¥à |ý@;bÏÃøÀ;7šr­™À<¨©Û0=@ÄøqÁ8o?þ#¨FÇ?Ԁ#[¤Ák?äê<ŸB¥í@SÒz‹·Y?ùQµ)mÇ¿ïÿû˜'2?ïÿjÕþпÂÒ練'8¿êRz᝔P¿ç"Ü0¿ïÿ(3û°AGNbcu3FGL J1528.7-2247NVSS J152834-223522?ïÓÚá@)ï?‡)MÅõ[ü?vTìHm?‡)MÅõ[ü?ê^$1§[¾?ÂÂ%X4?Ƈo9b'	?ÂÂ%X4?îBr"¥?™çñ`©?«ÞÓF
<?™çñ`©?ì•ýsf]?Ÿ'[Ôëhê?»WØdÍ?Ÿ'[Ôëhê?ï³IÇ&ù?ƒÚ{ˆúÌx?ƒ-Ž,úÇ?ƒÚ{ˆúÌx?Ú/ÕÙnyc?Ñxg$§TB?âèHÃO?Ñxg$§TB?ë駃…?¨"§¿â?À[…cùñë?¨"§¿â?áD2
­ò±?ºkëû*?Ýw›ê¤ž?ºkëû*MIXED4FGL J1529.2+3812?Ù¾¢p5{@K¤÷<ÉÀ;ŽõѨÕÀ<Ò¨Rcz@^{/v:D?ÿ͕I¨À?Ég=üºÑ"?ÁEûø3'ä?ø"¸vÔr³@Ë܌ÞJ¿ïÿæ¦Sf?ïýWÿ›V2¿æ3߀ƒž¿Ú
˜à66¿ÝÒ	L¯Ûû¿ïÿûbâMhAGNbllNVSS J152913+381217?ïüŅR1H?3Q-Ár?9ÓÓt¯Eþ?3Q-Ár?ïâÒòop?p®Ў1‹?m-
R™—ü?p®Ў1‹?ïÕ`²ÐÕÏ?w€Zä–-?uO¦VÈ?w€Zä–-?ï½r~øƒŠ?d†wäú&]?€£`Oõƒt?d†wäú&]?ïïFž8Ôw?`ÿ³g=¬T?`¹aÀLQ`?`ÿ³g=¬T?ï"bÀÓ?›æØñ~?ŽçP?›æØñ~?ï¬òΩ?…†·!'`•?"Ãx»'³Î?…†·!'`•?îhm§£H?"ÎæÛÖOä?§	y&a²…?"ÎæÛÖOäAGN4FGL J1529.7+6733¿ï]>ù©¾o@E 'RTaÀ:ø+ìïÀ<Ú]^è@#f½ú!@ÕÓ;{×?Ä:Ôd¬R?³En߆¸Á?îï–ü0g§@•ÀR@Á¿ïâwú ø?ï5Y³Ð|…¿æíUj• ¿ãËЮٝ¿ßÞÖd¦à¿ïÿ€ß֕AGNbcu3FGL J1529.5+6733WN B1529+6741?ïþÆ9S;?±¹ØD5O?#Ÿ¹/
Æ?±¹ØD5O?ïö'"×?U¢)$ž"?SØû1?U¢)$ž"?ïìM>)äÞ?`$²h§Ç?c²ÁÔ»I"?`$²h§Ç?ïóY¿ö
ð?A­ÒXvg|?YL w@î?A­ÒXvg|?ïý^Š¤ß?0{ »?5ª›t~ˆ?0{ »?ïÖÑ[ZwM?yÜ.†Ô"¢?t—Ra2µ3?yÜ.†Ô"¢?ïÜ¡izJ§?xúoÓ?q¯K.=a?xúoÓ?ïşÆH=?mòÇ=¯Î?}0ÉSŒj?mòÇ=¯ÎAGN4FGL J1530.5-3026?ï¹(Ž@†@5öè)I¥À:"¡°¿P
À<IŠÃ=@ Ûà­T@š¶ÐF?Æì,c‹?º?Á¶Ašÿö?ý,…]T@˜%Ùç½?îåA7Ø´b?áuD C¿ÞA&¦\ö{¿ÛìVÀVë¿äUÜär¿ïÿséèwAGNbcuNVSS J153041-302559?ïùÎSTI?Aµa¾?HƲûÄ×?Aµa¾?ï˕þb#¿?'ðœÌËë?z5®¡Ì˜?'ðœÌËë?ïèÈuœ†«?qûa|Fƒ?g7Š4¾¤ô?qûa|Fƒ?ïÉi/eë?`¢±¨©Œ?{Kh9|É?`¢±¨©Œ?ïîÜÿA`•?\Ž"^­J?a#öùÏ?\Ž"^­J?ï´5ñ?­c¤v3¼Z?ži<Ï}Ò?­c¤v3¼Z?ïÜñgya?xð{&¶¨ì?q‡pQÄ?xð{&¶¨ì?ï&FŒ"Û?…ëW)ò·?›>7%䞮?…ëW)ò·AGN4FGL J1530.9+5736¿ìL©€0UÍ@HUŸ<pɗÀ:¸Òñ±‰À<̋Ջ¸0@$֐šíW@8‹aÈqô?½+¶g/º?ž.–¸¶ã?âTæA?ýS$Z'hÐ?ï bb ´¿ä	£ý˝M¿Þ†\㔏¿äí·(Ùº¿É$û(Õ·¿ä+4̐fëAGNbll3FGL J1531.0+5737WN B1529+5746?ïù¢MAÅ?E™YÆW?IvÉð­\Y?E™YÆW?ïò"cð?X\Õ
¹b|?ZÙù¼µ¦?X\Õ
¹b|?ïåÒDž²?rŸ–Ã,c?j-8JÞÆV?rŸ–Ã,c?ïÕ}üÁBf?]BòܔŠ£?uAºÛ¬»?]BòܔŠ£?ïíòûW?^ßâQ'²?bû°e?^ßâQ'²?ï̖Z@B?|F£qÄqi?y´ÓüFÙ?|F£qÄqi?ïèÒe׺?vdT›ì?g-šfø&?vdT›ì?ïHŸ7Þ?"cêÌ?–ìŸù8?"cêÌAGN4FGL J1531.7+4710?à0w'(~F@JpÄÑ¢À;:›!YÀ<çK,N<¤@dªrÚ½ü@ƚƒ¤dÏ?Ä[}i¸*~¿—ïY¥ÉäÌ?ÔsæÂer?ó݋s¼e?ïf[~«Ø¿ìB¾$=w¿»òRÃFfA¿ãŽc¥ÁÆ	¿â?~e`¬é¿ÓS'úð̆AGNbll3FGL J1531.8+4704SDSS J153139.78+470705.9?ïõç†È˜?Z!	vᇿ?Uô0É3€¯?Z!	vᇿ?ïÞ­sQl•?vR±sm?p©Fa˜‰??vR±sm?ï·¬‰WÏl?"Æ÷!"b>?'ݚíÝ	?"Æ÷!"b>?ïhŒ´Xã?v€ßC0ÿ?'ý.g½¯?v€ßC0ÿ?ïð"§0?],˜"â
?_Ëjú°B?],˜"â
?ïbjŸÊÏá?™+¼'õˆ?"²¬ÍmÐ?™+¼'õˆ?懶‰ÒŽ?‹r\¬†b?†Üˆ
@Š?‹r\¬†b?í0ý¬q@=? €<'°àì?¶x›š? €<'°àìAGN4FGL J1532.0+3016¿éqŽ–Â_ó@Kh'£"¯À:ܵxqÀ<\…íë*†@ÐÒ=úâ_?þHH¦4?µ¦â­^Èb?šrFQэ?ä‹Lš† @	'öWµžˆ¿ã¬,ÿ<‹¢¿Õ¢Ô€ËA‡¿à=Œó˜ép¿×®Ué@ Ú¿ãyˆíyë~¿ÝÑLcZî8AGNbll3FGL J1532.0+3018RX J1531.9+3016?ïþ'òWî ??þ¿DÞ¤?&ÐÛî'±‡??þ¿DÞ¤?ïösçOÒH?_iäa%?S1½ÐÐ$?_iäa%?ïô†s2bå?U.+›ì"?VóÒ3õî?U.+›ì"?ïõ"USˆW??õK€j©?T÷Ul-!º??õK€j©?ïü‹o›‰?2šLÃì?;¤"twƒ?2šLÃì?ïÕ·Læk7?z,ž"¦,T?u$YyŒ""?z,ž"¦,T?ïõ¶þ"Tä?amڛcë"?T'T˗Ä?amڛcë"?ïè½ûí?V˜ð²ö.?gBû,?V˜ð²ö.AGN4FGL J1532.7-1319?¦ñàœ@@Û$Aþ¨À7éï®y$¯À;iTJ0@½†QŒ@‰~Ü~ñx?›D§¤Ê$Q?º(žYÇÇ@{•"d~@€6ŹÞ?Ú¡½àåοÜü""+É2¿âc[Ÿc6¿å
î \+z¿åTw·¿èÖÍÏ2ÙAGNbcu3FGL J1532.7-1319TXS 1530-131?ï»éúsèÊ?°¥
ÂÏéz?^ŽO"?°¥
ÂÏéz?ïâk6§(p?ѤIŒ@?m"Ép4è?ѤIŒ@?ï'1ª`Õò?Ö}Î؂È?s•n©»W?Ö}Î؂È?ïþ\@À?"±Óòl·?*;ðÜú~û?"±Óòl·?ïð"oÝ?[ÌVb;Ï.?_÷e–v"?[ÌVb;Ï.?ï€äÌb…? {.UÒ×?ÆÌí(îÔ? {.UÒ×?ïª2BW?‹¤^àb?…so"	sù?‹¤^àb?ïú'Žså?;²õ '#F?E»îDLÉ?;²õ '#FAGN4FGL J1533.2+1855¿âY‰fE¯7@JóFí$À:Y-2h2À<Y´E‹@ ú$…ñF)?ý
fóT?¸CÀ°E¿–¹Æ_ËA²?à'ß@lך?ò,{Þó•ä?î_8	[ÉT¿ä3"âz´¿àù&ÝdtŸ¿Ý…¥;8eL¿Û¢†\ûـ?•_m"îžAGNbll3FGL J1533.2+1852RX J1533.1+1854?ïä+ÒR?tªæ†¦ß"?kÔ-rã¥?tªæ†¦ß"?ïÆñhãnO?†·83˜Ì?|‡K…Yܘ?†·83˜Ì?ï…Ëî¢×Ó?r3]¬VÖ?Ž^)C*?r3]¬VÖ?î׬àÚ\?ˆÙàº%?¢…1îê¢Ù?ˆÙàº%?ïÁoaކ?~ø—*‡??HOZtUh?~ø—*‡??îdþ➛6?²óâP2Ú?©°ÖLž?²óâP2Ú?HæH?½šì«?Œm¿š6?½šì«?ê–r:ã‰Z?­æ,r¹UÙ?Ŧ7qږ?­æ,r¹UÙAGN4FGL J1533.2+3416¿ÐI°fÿW@K\
è³³À:4nµÀ@ÍÀ<tݒîY@úŽñt÷Ï?üo[Ømë?¾Q™Ð¡?»Ê³íض?ÿwÑȵ@ǙÚ\,|?ïö&' ®·¿àׇB_ ¿Þåqúfä¿ÆcGãnyÛ¿æ+iÀú)¿Ù=Ÿ¤u–AGNbll3FGL J1533.5+3416RX J1533.3+3416?ïüOUl‡×?4C~*ªŽ?=…S]ÿ
?4C~*ªŽ?ïîÂO	Aa?cÔ_ž7?a=°ïßfü?cÔ_ž7?ïêNÞ	‹?r´e…ê\ú?e±!Ò¸÷?r´e…ê\ú?ï™þ헃Ñ?i|`,ÌJ÷?‰€D¤mß·?i|`,ÌJ÷?ïõèIªî×?OZ?T/ls("2?OZ?ïÄGìcý?»ÖVú'Í?}Ü	ìíóq?»ÖVú'Í?ïÎÖ|¨È?ËÑÜÍg$?x"ó_è+Ñ?ËÑÜÍg$?îÜýÆÀ?‰—†Ï$†k?¢0.dú?‰—†Ï$†kAGN4FGL J1534.8+3716¿ï|Ç(žâ@K"^þ"vÀ:†®û*®)À<{¦_z¹Û@ -¤f&O @h	¹½%?Á…dXo,ß?tWíÞ²€Û?¨üð-¢P@®?aê«°¿ïþöë"Gù?ïû³ÀsQ¿çác'Å>¿ÚT°ÜVW¦¿ßaÿÏ¿Ü3oce*&AGNbll3FGL J1535.0+3721RGB J1534+372?ïþ†Çô£?>%žþ6?'""¹÷m.?>%žþ6?ïö4&o¢È?X ò…mc˜?S—³18Ï?X ò…mc˜?ïõօՎà?UšBª€6é?TRóÛð`?UšBª€6é?ïø/'	Ÿˆ?8ºDy
?OA»¾'»Q?8ºDy
?ïý[Òÿ?3ÉV%#vj?5#yÌD­?3ÉV%#vj?ïݶH{ð?tþV6!=?q¤æÀÈ?tþV6!=?ïñ#?Žúô?nVÄ~š7?]¹c;gv?nVÄ~š7?ïèÃ=p¾?\0–Ì»Õ?gþ<²"{?\0–Ì»ÕAGN4FGL J1534.8+0131?ìq½~ór@Ev¼ÿ À9‰èK®TÀ<½ÅÈ̍@ÆÑÄÙ8k@-ú¡ò-¯?©ã,›Ð'º?¡‡ê<ÒG?ó-ø–2æ@:ñž"S"¿Ì¦bÀi'¿ä­ºþ™"¦¿æRÎÙíFÀ¿åù?¼ ¿æneÆ-¿àËVq_iAGNfsrq3FGL J1534.5+0128PKS 1532+01?ïü_4v‡Ï?>bé´Á§2?=[½ë@?>bé´Á§2?ïôDú?loì)ª£?WÑÿ¿Më>?loì)ª£?ïÔä²,ô'?}g4=z;?u¦ØW«Ÿ?}g4=z;?ïÿd°e…?Qßwãïs?AåÜV?Qßwãïs?ïýP?.'}¢·?1ïã±TMø?.'}¢·?ï°Ð
!Ÿ–?˜mR\Ñä¥?ƒËýƒž¼‹?˜mR\Ñä¥?ïÜÝÅ(Ͼ?w£I;KÆ?q'‡Å?w£I;KÆ?ïÿ'cuE?>ªà3Ž?tdz?>ªà3ŽAGN4FGL J1535.0+5320¿ë[W(ÆÙ@I;:h²À:ÙUvT4À<»×¿o8@ ¥D#ñL?ú¿Ãvâµ?Æ»ª¦ds?ºs欜֐?ôŽ¯«SÖA?ú3–b'$¿çª=UËä¿âvþèÓ¿¿ãOb2Ôi¿³à}:"¿ãc܉ٿÏ%ï¨ÄÚ»AGNbll3FGL J1534.4+53231ES 1533+535?ïýÞAB"?&üo v€ƒ?1
öÈ3??&üo v€ƒ?ï珜ÑÓ?h>%O{Ûq?hpc>º?h>%O{Ûq?ïî2—Ï6?o)›üÀ›i?aÍh
MßN?o)›üÀ›i?ï¿?4둀?b|jçÛî?€02Ë¢áÝ?b|jçÛî?ïüºe8‹Y?2ւ3ëÈ?:,ոͰÄ?2ւ3ëÈ?ï£vÌ(ü½?‹¸´
¤ˆ?‡"M@œ?‹¸´
¤ˆ?ïñúVí!?oÌe:Ê?\T
ÝîL?oÌe:Ê?î½t8ÐÅÅ?%…"™?¤(¼ró£·?%…"™AGN4FGL J1535.3-3135?ïý­¾¥ÓË@3z'Ä"BhÀ;IØ›ïµÀ<"ü4µê@!¸îžƒ¹?üÁÃiv¼?ÔKí~ÉÈ?ÈIW·Ìàn?÷:Y²ù¼ð@¤Ç¦È+R?ïʺŸ¹¿îegÞ`ú?Ö»&F»¦4¿ÉÌWÇg2>¿æåöŸ..¿"ì Çm3×AGNbcu2MASS J15352963-3133461?ïþ}—c%?˶YT³¼?(&‡ü¼Là?˶YT³¼?ïàg_úU`?À7ö`ùÑ?o˜ ©_þ?À7ö`ùÑ?ïìÚ%rLÆ?`3FCPJ½?c%ڔ'qþ?`3FCPJ½?ïõį5Ñã?@5€5TÎÄ?Tv¡]bz¬?@5€5TÎÄ?ïÿ"®Ñ˜?å)œÙ;?͑,šÍ?å)œÙ;?ïL9G°~õ?§*£ôd¶ü?–x×8Sq?§*£ôd¶ü?ïã¢ÛÕ?t)QáØI?lñ]GPC?t)QáØI?ïâÊ?aZAâôç~?màoâÖo?aZAâôç~AGN4FGL J1535.4+3919?ì5¥NÂR@Jøââ¸Ç\À:ÎNCYòÀ<½'_Á0·@–À©ÓÎ@çÚaàŨ?Ã#¤õÃ;)?ÅÃ[Ÿc6@S,ÀRk@m‹¿ï‰«zl­¨?ïý_Üßiˆ¿ÝsÃüČ7¿æ¼þùoÿçdÂW(¿Ú¬‡]ðAGNbll3FGL J1535.7+3920RX J1535.4+3922?ïùå¶Êú1?Aþ¼–œ?Hi%JIÊ®?Aþ¼–œ?ïá1"cÛ?uøe]y:?nÎç~[Õ?uøe]y:?ïØØRå?oâRu沌?s"øô‰±o?oâRu沌?ï—	dÝ%?k1	Ë sj?Š=§	׊º?k1	Ë sj?ïÜ^6…çÐ?p¼'$÷¤?qÐä©\6?p¼'$÷¤?ïsǼ¹ý?£Î߃€?'Ÿ'Gøe?£Î߃€?ï,AúÖ?"únƒ†ÖË?šwÀ¾½
¿?"únƒ†ÖË?íÜÄ{'é?œîå"‹?±Ü"&ܾ?œîå"‹AGN4FGL J1535.8-4730¿í¾iƒë÷#@Ô
ª}íÀ9òż7SSÀ;YË0ëZW@ÙQj€Ò@'þ?5Ÿõ?ʌ×ÿ°ÏÁ?ºŸlÂK¥?ñï_˜@Ê.¿çk(¢¶xÍ¿á­|5Om¿é
߆ã´p¿åd±û.·¿ïývƒ?Ñyé{VwAGNbcuPMN J1535-4730?ïüS
Þ)?<[Қú×?=gxUÞ¾‰?<[Қú×?ïÚd4°?€-™Ý¶zã?r÷Mï—?€-™Ý¶zã?>‡G»?{i®
eÚ?€Ø^9góä?{i®
eÚ?ï÷+)hH?@€®Yóö?QÓ©e·`?@€®Yóö?ïû‹}L1?JšÚCž«?C­Ò³•¤—?JšÚCž«?rQ|?³Þö@\¾&?¦Å¨Þ^"@?³Þö@\¾&?ï	G
Iƒp?"Ù¹^`'?ž×Vϑð?"Ù¹^`'?ÿۉ?'ݯ¢2X?Œ]@*›Ç?'ݯ¢2XAGN4FGL J1536.8-3155?ïþm•&:@3…7âÅ]À:˜0òçÉÀ<MãÕ'b@éÿð:»@nÅý0B?Å ¦ÿÝo?»17°pu´?ù»aj~#@ý«Ï§º?æ§,ßÜôã?îŒðÿ1#¿ê¼'ÂåÃ>¿Ëùt`$-¿èû,=WN¿àm­'"ªAGNbllPKS 1533-317?ïûv6¤=?:-—®¿£…?B'$Å+ªp?:-—®¿£…?ïàk\¢÷?xç
Ý4?où"'ÞéT?xç
Ý4?ïÂbÙOM?wk€ßh?~ôNŽˆå[?wk€ßh?ï붾(ÖI?K¬\€;Ö?dIApG?K¬\€;Ö?ïåçÚÑ?mUðF¬f@?j<Xä†F'?mUðF¬f@?ïSì!Œþ½?¤YIRœiŠ?•'{Î`(g?¤YIRœiŠ?ï>v3ý¢G?— j°W^&?˜19ƒ»S+?— j°W^&?½Gb"?yví†Ñvó?ˆÝœùS?yví†ÑvóAGN4FGL J1537.7-7957¿àNu]>
qÀ3rŸb0wÀ9wJ‡ãŽ°À<þ–µº@Cƒbu–@Òâu«}È?±	]Ýçãe?›Z*‡¬Ëê?é´/JWè@'ntҺͿÆzðv g¿âCF;M³è¿å¦ÃMÈ	ï¿Þ5|c¨Ç¿ç»ÿTßUf¿Ùa¶ÔAGNbcu3FGL J1537.8-8000PMN J1537-7958?ïþ"Š"?‰ø
o…?'¾¨xg}ù?‰ø
o…?ïöºŸ…}?T|'ª8Q?R‹×Dæ"?T|'ª8Q?ï÷Te?S‹U±©Û?QÃØgÅ?S‹U±©Û?ïûñj»à–?/"»û1?@:Tåœ t?/"»û1?ïý|
ΡI?(Ë×"`R?4ªðMT?(Ë×"`R?ï×·V$?€ªP8æ8?t@$u¼­ã?€ªP8æ8?ïô†è<?c›Ú"ÏìÀ?Vò/⍪«?c›Ú"ÏìÀ?ïô€nê_?I–g{àYE?Vÿ"
´²?I–g{àYEAGN4FGL J1537.9-1344?à˜"LÅi@@EæšÔ,=À;ý>" À<u¡gÄ4x@!ë¨îv?Í?ù6 hUSï?Ïô	Q¸Yx?ÌfÜX$­@WƐr©@ùìðٜi¿ïÿøsCÄ{?ï˜b'p?ïß°Ÿoœp¿¨îi t)¿äŽ¸Ê·H׿…ž:J…AGNbcu1RXS J153757.1-134334?ïþ#ý"Ǧ?%¦ðP˜3Ú?-À$¢*?%¦ðP˜3Ú?ïåՙû?xp2"Äð¿?jê*qëÅ(?xp2"Äð¿?ïÑnvoë?xû'!—×?wHÄévJ8?xû'!—×?ïÞ‰`!º?`ã˜4¤€]?põ»6')?`ã˜4¤€]?ïþÐi~7­?#kÉ R«?"ùg¡îk?#kÉ R«?ï¦Ïò"}B?''dz?†LW±t?''dz?ïÔ~–7?yãˆ8½È?uÀüÑ°?yãˆ8½È?﵅ìFBb?wyø®˜Õ]?'ž"êOßz?wyø®˜Õ]AGN4FGL J1539.6+2743?ï·Rñ$×@Jnž²gÇÀ9‡tw¡!MÀ<^c˜UÌ»@c"çQ@…¨¸ñ?®ŒÕ;d™?ŽÐ¸rwÂ?Û@ï~¨|‹@Œ+.,
O¿Ý UàÝ%
¿á±ˆmø+¿åc(>«	¿ã(c@Â	¿èQ¥^ɹó¿Úñ VL<ïAGNfsrq3FGL J1539.5+2746MG2 J153938+2744?ïþkQÃ?ó§ñT­?)Jòl‡îµ?ó§ñT­?ï÷_"A'?]SOƄcÈ?Q@ÙLTœÛ?]SOƄcÈ?ïMj[?YôæÎR?aTtz<
x?YôæÎR?ïÿ|‰µÃ=?°¯zs²m?nƺìÊb?°¯zs²m?ïû{ï9´,??IÜþÀ™?BDÒ?™??IÜþÀ™?ïًv,ú?€Xrþ¿T?s:E‡*Ò?€Xrþ¿T?ïØaÍ>PŒ?x^«"ha?sÏtÅu¨?x^«"ha?ïÿVݾÚ?5¬€<Ã]?<ç%DQ?5¬€<Ã]AGN4FGL J1539.7-1127¿ïˆ3´ØÔ@@ëˆe"¯OÀ:!4–àµÀ<"ý2Æ%ê@ çTWÆ™?ü¨Ö¸ÞÙ??¾KÞ'ñ?¯|©,?ñ¥×Ë-\@œ‡VKJ¿îê´^–ä3?×p6~—4º¿Ó3ƒ$¸:¿Üã'ìý¿Ýt ƒƒ,ƿفí`@1žAGNbll3FGL J1539.8-1128PMN J1539-1128?ïəÁT"?²epŀv_?{3fsŽ¯?²epŀv_?ïé¡ÃB?v¬,C¬ßf?f^ó2Ýã?v¬,C¬ßf?ïݯli¶?|V(
æ¼?q}(*Þ©X?|V(
æ¼?ïçý(?Q™ØùÙ?há¶Ý¯ñ?Q™ØùÙ?ïøù¢²‹È?M±<?Lu\Ù=´?M±<?E.n?›ÌBrEV?‹î£6Pt?›ÌBrEV?ïÓæ#,wO?}ò˜ûòNÆ?vîHÈÒ?}ò˜ûòNÆ?ï ¤vê?wãÈQëî?‡Öúö¦A?wãÈQëîAGN4FGL J1539.9+4220?á'×]Ÿ@JTøœ^oøÀ:ñ/!U»À<·Ö™Õ(¼@BÉ0`@ÞKÊÙ­†?Ín
å÷R?Ò¹·FRË@Ü$Ts@ž‰XöU?ïú	Iú¿àì5]YøD¿åÑ,½ùf¿ãVq_i¿ì˜FÉ))¿ïÿ韖]ÐAGNbll87GB 153741.6+422719?ïÚ0³¯¢ù?jхŠkBâ?rç¦3-Cx?jхŠkBâ?ï»ó$""Ñ?'¼Ù.kã}?6ê"«?'¼Ù.kã}?ïV=qÙá?‰ªÀ¾âü?•8QÃ%µð?‰ªÀ¾âü?îæ±>É5á?€¾•°`š?¡"ì!ø?€¾•°`š?ÌV
?Šà»ª=>?ø;.?Šà»ª=>?î‹Ûÿ«Ør?­+Cý::Õ?§B@Ö-â?­+Cý::Õ?íÂÙ»À…?¢oâ"!ÀÎ?±é2 H%Ý?¢oâ"!ÀÎ?ê£bMRQ?¦¹OùYÌ?ÅrvÊ·ž½?¦¹OùYÌAGN4FGL J1540.1+8155¿ïŸÇþSO@@{w¯d:À9 *aÓY¯À<ýÎÍX
@  óS
?øÑäcÂG8?±Ò-÷ `?µk½AX@>J`vb]?ÿØ&,dŒò?ïÿµøtñD?¼(ŠbÄñ6¿Ûh1AÁkp¿Ê.ÇΏ¿ÚØ4¿¥F÷¿Ðžñ;º–AGNbll3FGL J1540.1+81551ES 1544+820?ïóœ{ºû-?^–;6Qº?XÇ'H¶?^–;6Qº?ﭛ
KÍ"?—A¾&ÆÝ,?"™=sëï"?—A¾&ÆÝ,?ï´°%C¨Ä?€ C‹~Ñ}?'ÓöªöG?€ C‹~Ñ}?îç1ì¥ôá?t`L¸iº?¡Œá3èãú?t`L¸iº?ïíǨ³¾?Z·ÐËRX?b8ê!²Zm?Z·ÐËRX?í'3"³Ú?Ãa@fný?¶Æca…HW?Ãa@fný?ïkêHÕÿ?D­Aԇ?''¶à²h?D­Aԇ?ëÿpðFé7?¥K»Svm?À<>ä[#?¥K»SvmAGN4FGL J1540.4+6606?ìXˆùý÷+@E'8\gàÀ;	j²VÀ<'$»¡+^@,B(C–@§£áñø?Åӛˆ‡"Ÿ¿'êŸÛۑ?ÈüCŠOO@¾¦y&¥¿ã3ßá& ÿ¿âHA'O ¿êgÖX€u¿×^ä|káP¿ïÿk»9ýR¿äFù^PBcAGNbcuCRATES J1540+6605?ïü¤4tž??à3øÉVÎ??z܄ªJ±??à3øÉVÎ?ïö6íÊ?Ì?RžÛfZ_m?S'$‰¼÷¬?RžÛfZ_m?ïæOÊe
é?hz2¤)®è?i°5f»??hz2¤)®è?ïõñTBê?<û't³ï?TW­|¬¤?<û't³ï?ïù)g\?NÃå*¹?K·Z¨×|Á?NÃå*¹?ïÛG¹I"¦?sBrNÒ¥?r\#@p¹I?sBrNÒ¥?ïÛhÀw˜­?w"¤óÊ|?rKŸ±¥ÅÈ?w"¤óÊ|?ï·L¸ëD?sßhñí?';,Íý$?sßhñíAGN4FGL J1540.7+1449?æÄIäƒ*u@Hiˆ;£D=À:EÖL¨O?À<XÑӜʧ@äA:2@57¹«?·`éàêø¿¤$QÛ¦?×e;$C@úV6mzW?ïýÜ9QZf¿æýé¥K¿ä½`t#"¿ÞÉ«…)u¿á¾ÁqN÷µ¿é¨ü¾W7AGNbll3FGL J1540.8+14494C +14.60?ïû%Ž¦4?C£EBi?CiÈZ°·ì?C£EBi?ïôêWnž;?\óψ6W?V+P¬û9?\óψ6W?ïÝô4ù9›?x¤%>I?qåtDê¦?x¤%>I?ïåצ"F¯?Ps®×N?j(Y»]8À?Ps®×N?ïôݸ½?VÛ<"µ?WÊD£V?VÛ<"µ?ïʦséÿ?†mø'¯Ì€?z¬ÅísÚ?†mø'¯Ì€?ïÜýŠÀôã?{àëdªàý?q:ºR'?{àëdªàý?ï®ûþ¾Œm?o#-äˆ?"AI}¬¼?o#-äˆAGN4FGL J1541.7+1413?ÁmK®\ë@H,ü'œýÒÀ:ψ[ƒ´À<€©={‹'@ Œ«hy7?ý|=¸ƒj?Ë6¢Êê?¼»HjýÏÏ?òÆ.jÑ@ÐØ;Y¿â¸J^Èã3?ïôhAÝÅî¿à@ÝݖI¿ÛÜ\AŸ\§¿Ý`½¨"¿ã6«ÃgÉ=AGNbll3FGL J1541.6+1414WISE J154150.09+141437.6?ïýÿè-%}?'³Ê±?0½.0L—?'³Ê±?ïï€óIR?jh÷
œâ?`ªOJÉ?jh÷
œâ?ïêØ0á§Ù?g½g3%Ö?e'Î÷܇`?g½g3%Ö?ïÔ`Cã?Yª˜Ç€?uút7ÐÊà?Yª˜Ç€?ïüõò¾Ž?1 Mç©ü?8Pl·ŒŽ?1 Mç©ü?礼HbM?°
¹^}?…ÙÿqWº?°
¹^}?ïäƒEW?wA04?kä|Ù|Øù?wA04?ïW¡ê‡?'ºGãé#é?•2¡ç?'ºGãé#éAGN4FGL J1541.9-2915¿íLnČj@4c†Â&€À:ŸBP©À<3bàŸèh@ h ¢¢V×?ýRÎ8ݗ?¹íY	[ža?¹+œïÑà@¼íƒüyc@°|OG'?ïæ'P¡Ù¿ÖWÀü_©¿Ë߬bôìÑ¿Ôè#ëA­¿âüæÛkÌ¿Ù78+>AGNbcuNVSS J154203-291509?ïûàÔÁ]?5Ž<õ'Ä
?@|¯'ã''?5Ž<õ'Ä
?ïÄü\*?‰°¾ÿM¶?}õ0>ÇF?‰°¾ÿM¶?ïðdÉ«?bËKRñ·æ?_ù85߉‹?bËKRñ·æ?ï¹<›«†p?c¢¬©
?°ÙgÖ?c¢¬©
?ïöb£¹-?I^ú¡¬×?Sß:¸¥›?I^ú¡¬×?îç	V•ãØ?®t¥É
?¡j˜Y†?®t¥É
?ïå±êÀ ?u"%z¥šÿ?jNnŸœ?u"%z¥šÿ?îúU•‡?† îòºÃ? Z¦°&¥'?† îòºÃAGN4FGL J1542.3+1801¿å^ÉÌ3Â@HÜ#|ÜÊqÀ:¦µ{wo£À<\š¨Rc@ù¦&oÖ@ ,ƒɖ?ËhO_8Ê¢?Ïÿâù´âJ?þ‹¾z#²@	Öv·Au@¿ãµ>p~]¿Ùãàd¯,¿èh‰ø;æ¿éç§^~:™¿îRËI?3¿ïÿ2FÄàAGNfsrqOR 167?ïñHtEL?Xy7F,1?]oͅhæó?Xy7F,1?ïíþ%4lï?háïW<?bÛ쨛?háïW<?½³1ú?ƒU ײ¢3?ßЈ䭤?ƒU ײ¢3?ïÅö#)È?c®UÂ?}îUq°?c®UÂ?ïðà¼)!É?[ȺVG?^>‡:I…?[ȺVG?禮–29—?Žüv¸·úª?†RZ}ÀnF?Žüv¸·úª?îÛ5DÒºD?–Š6/÷E?¢L«·Þº?–Š6/÷E?îvÿ­Â?"¹ãÉ»
Þ?¨$ºÆü?"¹ãÉ»
ÞAGN4FGL J1543.0+6130?Úyi†_Ö@F°üø
Ã7À7‹g‰|$À;LãGb•!@ Ï6K?þdØâ"Äö?•#VØe˜?®vý@Ã@•B½ò%@
˜™êL¿¬"'È¿ÙK'àD£É¿ß´`¥_@¿Þ–ÖZ²Ô¿âÌdȵ2¿åcܺí§AGNbll3FGL J1542.9+6129GB6 J1542+6129?ïüDA+??T]v]4ž?=ßÏVDX??T]v]4ž?ï섖/àK?k3-Èpâ¸?c{i¨D=+?k3-Èpâ¸?ïÛ‰ú"?{ìK"™ƒ?rx;ÍÂ?{ìK"™ƒ?ïó$k?G¤n©ÑeÃ?Y·Ï­,i…?G¤n©ÑeÃ?ïú6'Pc´?D§±ãòh?G%»P e?D§±ãòh?￶´æÞ?†ìÎVë?€R¶Xޓ?†ìÎVë?ïÙf]N‡?€†ÊʕK?sLÑs‰gX?€†ÊʕK?ï×ø.ÐM
?dlŒq›)c?tèw'3?dlŒq›)cAGN4FGL J1543.6+0452?î™HôÄL@E¯àŠï²«À9ð³!*3À<,œ \–Ú@ {ç_u0"?üxœ‰8#?¼W®'¥¹?²á°^­	Ž?ù(¤Ð.@
nòÿ'p*?à8Q_îýú¿è*<´¼4Ï¿áÄö¿w'¿Ô¤Vg®æ¿Ý˅å\»˜¿ßÚD.®AGNagn3FGL J1543.5+0451CGCG 050-083?ïþZLWê?Ë-­³àA?*_Ù¾¦·?Ë-­³àA?ïòp Š >?g.f—§²?[¿`òô?g.f—§²?ïñãœ
üÍ?bT"‹U4?\8Èe°?bT"‹U4?ïñWN#,?A5'1Ô¿–?]ÛPí‡??A5'1Ô¿–?ïüÃh'º7?1Û"`20Þ?9ä¾qê?1Û"`20Þ?ï¡ìpÎk«?˜ü¡?š
¢?‡"ãÌeP?˜ü¡?š
¢?ïê€{TMú?rSôtâ¥?e"Ç.æ
?rSôtâ¥?ïÙÕUKOÎ?]½Trg¸`?sUnõÀ²?]½Trg¸`AGN4FGL J1544.3-0649?îÁ¢(Ö°H@BŸ¸gÀ9%'œüûiÀ;њ#,Tó@ 1ݘL¦?üðI ]?®ÎdÒg–g?«i¾_¡¦-?ÿAVâdå@Nn|4"?ïñâÀÿäý¿Ç=ÈwþiR¿ÙŸ¹Ù«¡¿Û R:µ]š¿àÔ7ŸÔq1¿ÔåÓc¿ÂùAGNbcuNVSS J154419-064913?ïþ)¿Iµ?6ev¢z?-d¢B»?6ev¢z?ïñƒÇÉ¥?pSUuÑ1?\ù̑hõ™?pSUuÑ1?ï¤h¹–¨è?ˆæÓM`;?†åщ'º?ˆæÓM`;?ïÿºé¢_>ôjv7ׂÐ?}À瞬3>ôjv7ׂÐ?ïýy»¶Wž?=¡Ð«Ú8?42#±€ô~?=¡Ð«Ú8?ïtO‰!Ÿ?¥JIÚ|~?'|–rÒ?¥JIÚ|~?ïŸ8-\É?>)±TK\?ˆ?qíɕ·?>)±TK\?ïÿÐlvl>óáut7>÷ÉþYp1>óáut7AGN4FGL J1545.8-2336?ځ¹T0?@8ðgȗÀ:äì-»$.À<a`'÷–¥@"Xײƒö?øpDÖÉ¥Ñ?ў@}·÷?Æþ<"¿j?óYæ/tb@3Z™©‰Ò?Ð0ÿV·È¿í¢FF5nw¿âJßO0j¿¼R—|ˆç›¿×,àÞ§•±¿åï!öÊÍAGNbllNVSS J154546-233929?ïú4uÂ=Á?D×Ë;í V?G.(åq`½?D×Ë;í V?ïè9­JÑ`?q»Ø‰€v?gÆR³ÎÈ~?q»Ø‰€v?ïãM¯á.¯?l‰zÓ0ð2?l²P=
áB?l‰zÓ0ð2?ï÷5šä?;ðQy?QٖÆù?;ðQy?ïüë4ä/·?6UŽád?8¦W6îb?6UŽád?ï'!ä	?"«ˆì?‹w‡

Ü?"«ˆì?ïâő3ƒ?t9n)_&?m:nž=Í&?t9n)_&?ïÛ.Ö¤‰?eódÆfâ?r@h~°;r?eódÆfâAGN4FGL J1546.0+0819¿ÝÇ àö$Š@FVV>Ðö'À9¸ÀûÞ2PÀ<)µÆ 
b@×-¹÷ˆ?ü¢HåL"?¶íz—JßÍ?ºÀ‹J÷J$@J˜Yþy@…Éy±ì¿äz-ô/¿âDx4Å«¿ÜYˆœò®¿Ð™:¤É¿ã*T'8T¿ÞÊ^=M'AGNbll3FGL J1546.0+0818RX J1546.0+0819?ïûò§|Ü?2咊{?@5a
,æÕ?2咊{?ïâó>ï?uœ Ð"­|?mëֈï?uœ Ð"­|?ïì;¶u®"?cFûD_ý€?cÄIÌIë—?cFûD_ý€?ï†eÀÃm?pµ´ž¼"?ŽfÜˆÙ?pµ´ž¼"?ï󋣕N?RÓ~Zä~ ?Xè¸VñBì?RÓ~Zä~ ?ïWGØè?¡!¬h¢X?•äþƒ?¡!¬h¢X?ï»Ø2Üv8?"[È8J—¦?	ó9>?"[È8J—¦?íÚR	?ÍS?–ùüWjOH?±-o¶oˆç?–ùüWjOHAGN4FGL J1546.1-1003?í"Y`ÛÒ@@Ó£"¯WqÀ:°ÐíÄÀ<1Y²"ý[@ bû0bsh?üqÖ¤?Â&ÂaŽæ7?ÄG0€¦Xš@ú¡ÿ™¨³@\ބ\?ït7àAØ¿Ùñã݊Š2¿ß^¡Ëí)¿Ô¤ô^N¿à½çŒk³­¿ã4…
š¶AGNbllPMN J1546-1003?ïþºMCT¾?%áúû¼K.?$[-‹Mã*?%áúû¼K.?ïñ)8'©?k­>ÝKx6?]­Ž¯ýi?k­>ÝKx6?ïéfüÁåœ?mX)¢fÎ?f™,<lj?mX)¢fÎ?ïýbÉñ?!°ú<Û?74ç¡Ì–÷?!°ú<Û?ïþ¾Ù2ûo?%]œç
ýr?$hƾ™ò?%]œç
ýr?ï¼õB•Y?‹‡;‡»W?€úB¬šù¦?‹‡;‡»W?ïÌâι-€?|['"°~º?yŽ˜ŸI·ÿ?|['"°~º?ïù'÷z0¯?9äC/ü?I´!͒qÈ?9äC/üAGN4FGL J1546.5+1816?Åþ"Ënæ@Ho"5ÒIäÀ;¦¸¦¥À<€rmæ@û•b'g@š¸–ž=?ÊçæٓZ?Ä2õö'Â5?ö+—]7@úx3ÃPø?ÂË>Ø,ý¿ÛeEÔö¿ÒZGòÝÙ¿ê\žÊù¿ÖäHŸ+(ù¿ïÿ×ñÃýAGNbll3FGL J1546.6+1812MG1 J154628+1817?ïȑTYQ3?¢nd¿JÂÂ?{·U²[&Ø?¢nd¿JÂÂ?ïïÀOÄl	?dŠôJä}?`?°nn.ô?dŠôJä}?ïÅ&W؄?x'8‹¾å?}lÔ0
?x'8‹¾å?ïßeÔxÆC?Sæ[¬È?pMÆ\Ž€?Sæ[¬È?ïºçòíó¹?†²pޘö?FC#9Å?†²pޘö?ï½<¹?†RÚMâ?€º0Õð=é?†RÚMâ?ïH6·;ü?ªYmJ)?–ù)!6†z?ªYmJ)?ïI®ÎpL*?"ìm½Lñ?–Ê&7äÈ?"ìm½LñAGN4FGL J1547.3-1531?Ã;x,©@=¬€ù£wÀ:ÛºÌð;À<kx(/Éò@!&öÝÂhp?ûTÙý6ø?Ô<Iý·{?Áõ:i³Lô?ò'r…X™õ?ù4Í\i¸U?ä¡ìï'{?çJ{NTø¿ßõ¯¯…")¿äÛî=_Üß?ÅGõâ𥚿åTh!§o›AGNbcuNVSS J154725-153236?ïþù"ß~?,²Ü²îÇà?.°iæDqø?,²Ü²îÇà?ï½Èö(Ã?'Ó¿Ÿ¥†?€Âl<çW?'Ó¿Ÿ¥†?ïÞ))p'?l°:P£þm?pë€E7?l°:P£þm?ïçõtIS?WøƒÐ[¯?h
þ TTÞ?WøƒÐ[¯?ïû¹¡Í?EÌs[óŽ(?Cã̿ܗ?EÌs[óŽ(?ï"Ԃg'¥?¯‡Ió¯ˆÆ?›¥o¸5U?¯‡Ió¯ˆÆ?ïÅk»Ô›½?}o ©š ?}J!ö¹¯?}o ©š ?ïwÖº­?ˆKYÏçúÊ?'(Á'Æ—?ˆKYÏçúÊAGN4FGL J1547.3-2802¿Çôµ7ô|Ù@4‹eˆUÀ:FäH•À<?,˜@ ¬Ùuҕ?ý¡ËFºÏt?½#Ë6I¾? ›_æ?æ̆'ø?øC®®(ÇÊ?îÎQfúàÜ¿Û'\:h‡¿áê9Ÿˆñ׿ÜÛÞaÔ¿ßS…
EŽ¿¿½¿¾œ]nAGNbll3FGL J1547.1-28011RXS J154711.8-280222?ïúåWs?9P¥]Ù?Dk¨ÉqHœ?9P¥]Ù?ᅦR'•?‡ßK½^=û?€:%,NÛ?‡ßK½^=û?ïçî_Tàh?o"TÒç?h   ×É?o"TÒç?ïÁœ¤Þ=°?d­lQèK?1­›ßè?d­lQèK?ïò<‹ ¯ù?R"ÚZ3?[†éK-.ó?R"ÚZ3?î¿mê¥a	?³ûì?ü"?¤	!Wa½j?³ûì?ü"?ï䩓ÈÛb?v¨þñu ?kVkýk."?v¨þñu ?îÖr –À?U¢¯Z½?¢˜Þ¶0?U¢¯Z½AGN4FGL J1547.9-6403?í¡³ßɇQÀþã'áïtÀ:†ƒ<`À;Å%ƺd@ò·É°b´@ßå®E"?Î
èuõ¥‰?Òþ¥¢fqÏ@ˆêb		"@ƒ&uµŽÃ?ï·Do›™N¿ã~Qª¿_¿ì&×¥mã2¿ãlja=1º¿ëcՒn,.¿ïþ|AGNbcuPMN J1548-6401?ïXô)và¡?™f"æTÔ?"ázԓ‡à?™f"æTÔ?î9sÉ,H?­G~	Ü?¬h϶ðz?­G~	Ü?í²dBíö? •F9ÐO?²lÝêO–K? •F9ÐO?îeàoc]?‰‰""¹éE?©®ñöv:?‰‰""¹éE?ëGù¾ÈR?À¢ªmð?ÃÆàÞ·?À¢ªmð?âô•iÅQ¿?Ðâõˆ×?ÚÕ,u\?Ðâõˆ×?ãYö¢Íä"?¸ê¡bþ·?ÙLºd6Ù?¸ê¡bþ·?àJÜ#EÄ?·Rn$s?ßjG¹twÃ?·Rn$sAGN4FGL J1548.3+6615?ïòä­$w@E0å£]gºÀ;—¸`.>À<Çç˜*-Ñ@bÿ"	•*@árƒ«Ë?Ãà|-Q¿·H"ø¦?ñrרÈá†@Kžuvy¯¿½;~0\"¿á³—!U<¿ë»G¿1X¾¿œ
F}Ë¿ïÿ¬ž5¿?ïýÝ`˜ÇAGNbcuNVSS J154831+661632?ïî¥|Ñ·Ã?]"¦ÛÀ?aZ'ìO½6?]"¦ÛÀ?ïíÚÓÖ?d0Ç>'?b%,)¿š?d0Ç>'?ï•%‹Õ¶«?ˆ í¾èf9?Š¶
'U-?ˆ í¾èf9?ïé`œ«zu?XdâcÕ?fŸcDjÒ?XdâcÕ?ï¤3ÁM"?‡dñ
¢??†þóÍc^?‡dñ
¢??ï‡ÈãM±?—þnÃG¶û?Ž
Ç#Ñ?—þnÃG¶û?ï­~]0?‡¯ìA¹?" h­Íßñ?‡¯ìA¹?î¸[lžu?›=ÛjºØ?¤zI:d2?›=ÛjºØAGN4FGL J1548.3+1456?ëÀ0'¡?ç@G˜–gµñ¿À8ú‡Š£\'À;É>»ýq°@'gh™ò?þ¼#1]p?¨FΤs?ºäÄæ#Šõ@uâXOL@Ý\ª%?ÞÏh=V!Ë¿»N®ä¯l•¿ÞSa;":¿áDÑöØ9¿ã^[`m~¿åÁ‰¢«'AGNbll3FGL J1548.4+1455NVSS J154824+145702?ïúÂKiŠÞ?Aî/"È?Döѕ'W?Aî/"È?ïì€c__?nÀ(ú͝?cœc©G?nÀ(ú͝?直ûêÐ!?…‹ÝVMb¶?…UÀ÷‡ì?…‹ÝVMb¶?ïÙ »Nm?Vó}"Û‰?s/ð øñ¶?Vó}"Û‰?ïûÞ7®B?6[;OÛ?@‡"OfFš?6[;OÛ?d/Ä-?šmK'Á?‡Û¦þ]ÈÆ?šmK'Á?ïÃN¾vj7?…LûvÒq?~X ·t—?…LûvÒq?ïzæ`Ð-?y)×p½øâ?£3ìٗ?y)×p½øâAGN4FGL J1548.8-2250¿ä—´¨@8,Â?«ºÀ9vh<)|À;ÀŒÒá¹Ä@ â×býÑ'?üâh?"z?¬Ï˜ü]* ?£'£Ÿæ?÷«&[´@
6¼ÕˆÞ?ïÿû-2h2¿Ì—Û´q6¿ÑWå.Ãaê¿Ù¥"Ï7á¿Üêö¦""¿Ô΄þ"?AGNbll3FGL J1548.8-2250PMN J1548-2251?ïþºH÷ÑÄ?!ÀY¡ó!?$[rߞö ?!ÀY¡ó!?ïîNÞpŸ?cŒU!¾@k?añ°øTÙ?cŒU!¾@k?ïê2œ›"?k*¢è»&o?eä͖>¤å?k*¢è»&o?ïó!Œä÷³?I¶ÓY#æ?Y¼åæY©Õ?I¶ÓY#æ?ïþP™‡?+™zt|¨?.F*€•Ú?+™zt|¨?ï?!d9ø?"k9ÙÐ?ˆ°7™32?"k9ÙÐ?ïÚd½€?€q!r§?r÷M¤¯"†?€q!r§?ïè…pJst?Z®'©2?gzë&sl?Z®'©2AGN4FGL J1549.0+7846?î¦p8'ä@Ahšþ§±À;çÿ:bËÀ=&(
á'@ ®ëA'v?ÿ³ø`îW?у¤D˜`_?"†`ƃ u?¼|`"Õm@¨ÊÈ»›!?ì¼]\Òi¿å­½Þ€i¿×¾¤kÚ¿Û逢&Ûâ¿ã;ýÂ8T¿Ø;Ä~AGNbcuNVSS J154837+784526?ïýÚ@LC?-5Q9¢Ú?1-þ)¶é©?-5Q9¢Ú?ïöÿ…~&?R–ÝjoY?RôˆàŽ?R–ÝjoY?ïÚ6¥-¡y?€õÍ/Fâ6?rä­K¢Ÿ¸?€õÍ/Fâ6?ïû/ø¯î_?'§(òÁ?C@ñ©ì?'§(òÁ?ïþñ–AÀ?@ŸÏ¶¨? æ›xä´í?@ŸÏ¶¨?ïØÜu¿ÓH?x³?ﳜ?s'Å1ôT?x³?ﳜ?ïî)â/=8?xs»'ûf?aÖð_/Ý?xs»'ûf?ïñjïjº?K÷›Gûê?]*!«½-Ö?K÷›GûêAGN4FGL J1549.3+6310¿ìZ")=@Eô<³åuÀ;NÊW§†ÂÀ<f<Àz®ó@Àe©}y@>Ü´¡]?»^ò>Kj7¿Â¦jŽ.@ô<¥¢¼X@¯:¥ÃH•¿ÖúüDÿìaðµà!=¿æô'¢TS>¿Ñ£ÌB¹8¿å€|ý ¿Ý¸ƒÕ6oAGNbll3FGL J1549.0+6309WN B1549+6319?ïþÍ%•ÄV?*¿ùö¸é?#-¤Ó¼6y?*¿ùö¸é?ïíò1"Ôf?eM}¦á*?b
ÎeLa¸?eM}¦á*?ïíö%I;?qI9-=èÓ?b	þ
ÑM?qI9-=èÓ?ï÷ܙã/T?Emåx"×?PFËÍà̖?Emåx"×?ïþ̯y2z?!eRQ	b?#5ç>ì¼?!eRQ	b?ï¡ý¨ü}?Œª­/|,?‡½œ Á?Œª­/|,?ïÖA*AÇö?{÷0…OQ?tßjÈn˜ã?{÷0…OQ?ïU;ÈÐ`M?'\ÙqaF`?•X†éc'i?'\ÙqaF`AGN4FGL J1549.3+4234?ÞAôuÌú‰@IsŸ©~+À;Z|Tå5À<ì¿\¢˜@awcä«ç?ÿÛãõhÍ?ɘÂçÇ?¿^Ðߚɉ?öH8c܊@\­+qÈÅ¿ï§î'‡Ù?ïýk›Y:¿â™ÝW‰¿ål妸f
¿Ë.×XìÖ-¿ì¨Ä¯ÇÙAGNbcuSDSS J154918.64+423500.6?ïü»XõÔG?0BPhr>ò?:%7ÑÒ°T?0BPhr>ò?ïí<Â0Å"?gøÿXVØ{?bÃ>s­A?gøÿXVØ{?ïãhôFt•?iÈrç}y?l—È©³2?iÈrç}y?ïé9Oµ}ƒ?Q̆'5G?fÆ°$ÜÉ?Q̆'5G?ïæW"ÞÁ8?mZ=@ž(?i¨k3¿?mZ=@ž(?ï°Z6"v%?‡—æ±½aQ?ƒérc	©?‡—æ±½aQ?ï¼=6Žª?í‡n}ú?€û°«}—?í‡n}ú?ïwn`}:¶?ƒN¦Žò'?'3î ÛM?ƒN¦Žò'AGN4FGL J1549.4+7409¿àâð7–P@BÜÿ—$tTÀ:¾‹ƒVa6À<±òeÊ@ Œ7Ü:S@EÖٖë?ºw¼úò¥¿®sìôQ?òæY¶T»C?ûn3´ãL¿Ù¢¥œ\AŸ¿åü†™Õ ¿êŠwB+ɇ¿ÒײÄbðæ¿ééâ‡I4ý¿ïþS!æÕAGNbcu3FGL J1550.3+7409WB J1549+7409?ïô$+е²?TVÌYþ*À?W·¨S•Ü$?TVÌYþ*À?ïÈH†à"?†そŽ?{Û¼sÍ"ü?†そŽ?ï³w[V=?~Éð§Üù!?ƒ:â'¬Å?~Éð§Üù!?ï—Œ,@?p>T]ª?Š<\ôïøî?p>T]ª?ïŽwú¸mo?‡¸çô´s?ŒbXÃÜ%?‡¸çô´s?î¸Ý31Ê?ª€þ黬$?¤r.­¨ÊX?ª€þ黬$?ï_Àž¯ó?ŒÜD}Í$$?¤?ŒÜD}Í$$?ë£ï'ŽQV?¬‰Ëúž?ÁpAµÆº©?¬‰ËúžAGN4FGL J1549.5+0236¿Ãèõ] Ö@DqÔbÃC·À9%[ÚjÀ;ümd‡i@ôÊöˆÞ@òÁmóùb?«ÂÑBÊ¢H?®Ú€Mœ@háa«@¯CWË[¿Õê0_ï(í¿å@ß=è˜Û¿ä¢i÷ë_¿äȖ<"¿ë´	tC¿ïúÓÍ$áAGNfsrq3FGL J1549.4+0237PKS 1546+027?ïúàY5j?=.»´tù?Eø~}z"&?=.»´tù?ïõ±-Æ?`™MtáT?T¤¢€'Ð?`™MtáT?ïÄH{¼0j?Íä²"?}ÛÂØ?Íä²"?ïû¶Õ>¶I?4¹¶Nb/4?A$¬	/°^?4¹¶Nb/4?ïö•Zg!?M
¥­ìµŠ?RÕJ»‹??M
¥­ìµŠ?ï¤Ò…‹¬?•êE›¥t?†Ë^Æ["æ?•êE›¥t?ï¹Ç´°?ƒMrÖ_"?¾Î;r«ô?ƒMrÖ_"?ï÷ª›kù?MÆïß¿¢Q?PªÈóÓ¼ ?MÆïß¿¢QAGN4FGL J1549.6+1710¿êxšà@Gä\ÈWóÀ;%–'~À<"íٌÏ@½³Wô†@'T·?ÁlIªC
¿¤ú [Ùß?åQ‡F°¾y@— t>Á1¿¶|n¨°¿èÀ*'_–>¿ãÐÂOpV¿å2Át‰À¿ÝËŸŠtc¿¯Öa"iAGNbll3FGL J1549.5+1709MG1 J154930+1708?ïþ''Û\?9ÃAr	?&í'ÊkŸ?9ÃAr	?ïõè¡-{}?]°Ñè§4?T.½µ‡%Ä?]°Ñè§4?ïò~¥L€6?a¡ø&Y"j?[µ³öÓ	?a¡ø&Y"j?ïüÌN¢¥\? ›g?9Š-·nW? ›g?ïýpaDœ?-Í8Ó?4|öÿwJ?-Í8Ó?ïÏV現?ƒà%ÊâãJ?xTŒÄÚ²?ƒà%ÊâãJ?ïó‹$XF`?cwzô\š ?Xé·Ë%0P?cwzô\š ?ïîÛÖ°7?T‡ÏãDÃ?a$ýM¹)?T‡ÏãDÃAGN4FGL J1549.8-3044¿ïâ"Ú#2Æ@2' d#–À:§$WÎ/À<h;¤ñ¼p@!"ƒZ=
?ûñLÞÕãÍ?Å/âç¸?¾l͞-ýê?ûŽÍ=5µ@f?˜ò)Ô¿¨è7Œ^H?ï³!ž¶9¿â[ˆAWŽ1¿Ò‰ÞÛÃ	Õ¿ÕJҌ)nŽ¿å-4±B-AGNbcu3FGL J1549.9-3044NVSS J154946-304501?ïü>*I]?5x|dfÉC?>ÆLóIl?5x|dfÉC?ï½K¶'!?†ÔÑ 0±?€­ƒÎsÆ?†ÔÑ 0±?ïîˆV·X?i³¹HÀ?aýwã®?i³¹HÀ?ïàï"*¯?Tèó¶Pø?olè–@ñ?Tèó¶Pø?ïïݸØN5?\üŒÓ"ü?`"Fø÷ÿ?\üŒÓ"ü?îËIág?°%·â&r¨?£Nd'΋?°%·â&r¨?ïç^—ÿª^?uÇ±‹z?h¡h´9r?uÇ±‹z?ïpk{5^?I¶bÁ+?'ò®á†A?I¶bÁ+AGN4FGL J1549.8-0659?ÕÌVÎݍ@A}j@ºˆÀ9=+úYÍÒÀ;ç<³åu:@ÄO(1L~?þ­ÛÛ]‰H?®ªq>lÞa?':Ǭ?ðÄ öð@¦®<éÀN?ï] Å¿Úó)âÙ¿âŸÒ}浬¿ÝT]¥L«)¿ÛÒ_qÕÛ¿Ú@ŽERš'AGNbll3FGL J1549.7-0658NVSS J154952-065907?ïüµQtօ?E·¦hÊwš?:UtéU
?E·¦hÊwš?ïë›[)‹.?q±¯ì'Í?dd¤ÿ°"=?q±¯ì'Í?ï؂:WiÉ?z÷ȏã?s¾â¼=×~?z÷ȏã?ïÈþaEÑ?e¸›ª7?{€ñ䪫7?e¸›ª7?ï÷Áón¼?Q7#w½G'?PÞ|‡€?Q7#w½G'?ï4OüS`?­Ž…z±?™vx¥ø?­Ž…z±?ï֔¡¸!?W¸¾jç?tµ¯*¿b?W¸¾jç?ïy-ȳ?}eN8AU?Ú_ZÏ–?}eN8AUAGN4FGL J1550.7+7006¿á6ãÝÆ«\@DjËGÀ;@öý»'À<º7ŽÆÞ@<Ÿg™?ò9ìxkL?ÛtiÉÈ5Ž?ïþMþ"7@O×^ FÇ@úL+&Ê?î¶Q•ôÉk¿Ýä©ÍÄC'¿âèj{€)¿ïg/ò?M¿ïŠÿ…†½¿à(6îÎAGNbcu4C +70.18?ïáÀO÷ö,?z¹Kw5P?n?¯ÖsÇ?z¹Kw5P?†V'?œ‹Éû Å"?‹\œ%I—w?œ‹Éû Å"?î:k9.?˜VH+ÕÖ=?¬YN±"?˜VH+ÕÖ=?îqtç*›?–z6Ö??¨è±¤U?–z6Ö??ïwû­?ŸH·©Ïòœ?'üüh¼o?ŸH·©Ïòœ?íå?1ÄQ?¾Z±Ÿõ©?°ÖtÖ÷?¾Z±Ÿõ©?녯Ι_?«ÊÃneu?Áé@ǁš†?«ÊÃneu?ì×ڄÆMØ?³
kèEï?¹A+קÏÆ?³
kèEïAGN4FGL J1550.7+0528¿Á~»7'Ø@EˆÁÛCÀ9œÊ
Õ«™À;ç þ}I@—÷û#Í:@,џšd›?´VÏÅzž?Ç÷Øi8'å@þ‹;26@
èØqÊ?ð¿ß'ü—?Í¿äD£""dS¿ãä'Ë÷º·¿íju>ÆdS¿í4€Û\²ˆAGNfsrq3FGL J1550.5+05264C +05.64?î¿qÿï~?£zçÚr¼[?¤ßüÄ%"?£zçÚr¼[?ï6j ?£°ðíü7î?™"Užsò?£°ðíü7î?í©ojq
? ø}jÝñ?²´"­S~»? ø}jÝñ?íö.PÜw¡?iHÏïÅ_?°NyBù?iHÏïÅ_?çã•ùHx6?Å߇hó?Ð8Ô
o"?Å߇hó?ê\n.ˉ?ÊJTgE"?ÇΎGDÑÛ?ÊJTgE"?âÛ¤šÃT?¹Èf>V¢?ÚäH¶ÊyX?¹Èf>V¢?äÝí[š]?´T¹€àR?ÖD%HäËF?´T¹€àRAGN4FGL J1550.8-0822?ïzâýÄD@@ól½˜|cÀ:ÏR]šæÀ<i‡¿}@!I³	,N"?û¬Ÿ¶Lä?ÒûOyx?¾G¼,@¥¸?ñaI["¤@/—b1ÎY¿ïh4œ¿¾Ç?ã#Mâáâ¿àYÕÿ{u¿â˜TTëꟿÂð@uœå¿áÍâ½ÐAGNbllNVSS J155053-082247?ïÿ5Ø݄Þ? eIL!†+?Dçô7Žâ? eIL!†+?ïé¬ÍAÖ?r̉eVâ^?f€Sáqª?r̉eVâ^?ﲏGÂGŸ?…ÁÉcõ?ƒ\.W²[?…ÁÉcõ?ïöãF`ân?>LkKÀÁ?R9s-½/?>LkKÀÁ?ïþ9H1X?;ùH&x?.ljÏ1oG?;ùH&x?ï¯Í–(ÿ?³X¯o©?ŸJNò®?³X¯o©?烈'€E‹?‹ší–@Ö?†X•ŸÉe?‹ší–@Ö?ïÜfאº?eÆU¯GøZ?qÌò§??eÆU¯GøZAGN4FGL J1550.8-1750?ïìp3Í@@;oyB=À:f<OšÀ<#PÐÒëË@üZ.Ì@¹cc}?Áꀘ@Ô?ˆ³xy¶
?Æúw•bÓ4@Šá^<K?ïÿ|ý¬"œ¿æ/N6ĸ+¿åÊWÂ^´Á¿äBÞ6œM¿ïlbäѦ?ã£æ#µèAGNbcuTXS 1548-177?ï÷ëX?N¹'a³Dá?P)OÏxuŽ?N¹'a³Dá?ïîĕŠ…?n`Œ®4?a;j…ùw?n`Œ®4?︦®;Mo?n8ºØÜ?ÖTf…ÚC?n8ºØÜ?ï÷Ÿ7#"ê?>¶õ"?PÁ'ŒÝ,?>¶õ"?ïõ*Mþ²ð?S÷;Š–ƒ§?U«c»"?Å?S÷;Š–ƒ§?ﮑ!ó<E?'Þ¾|º?"[·{IÔã?'Þ¾|º?ï¥E""¦?…( ®Ááò?†¿®‰ÉJ•?…( ®Ááò?ïÔ]~¥_?hHv©©Ù?uÑ@¼–e?hHv©©ÙAGN4FGL J1552.0+0850?ítJ®`6]@EӜZzÀ:E`Kš2FÀ<b«esø@Æ;óS?ÿƒ>Éijþ?À6+ágC?¿9òj@ƒaŽQ@	ZP1›®r¿êÒ×¾Bph?ïå
`¬B¿Ý™–ÿáL6¿à6çó™À0¿ãš¯ú./¿ê71Åté·AGNbll3FGL J1552.1+0852TXS 1549+089?ïýõ	"ô?&Çü®öj?0W±Ê-ʨ?&Çü®öj?ïì̛ñÚñ?o³)sÒñ»?c3d&â???o³)sÒñ»?ïê¼|G¤.?b¬ДÉ?eCƒÚ·é]?b¬ДÉ?ïÑs‡ƒŽã?\ѸGXt?wF<4™¦¹?\ѸGXt?ïö˜xºÚe?O²Ûr8j?RÏê€FI?O²Ûr8j?ï~mÌ¿¿?—›
k5?‹àdŒÐ,?—›
k5?ïÅÊý9Q?GNùƒSM?}ú€_D?GNùƒSM?ïY×EæWý?ƒõµ~"?"ÅJ8V?ƒõµ~"AGN4FGL J1553.3+0600¿íص]Ý	@Dù‰7KƨÀ;6Yì yÀ<"¬X¸þº@®qÔX²I?ý7÷¾?ÚWÌOðÙ?êPåË¡T@¹àF&Tþ@ËBhÛ5Æ?ÕÔ:ªJí?ï•÷¹	¡i?â+@š$¿ç²_ä@¿èÒGàê;¿ïú~¯"®AGNbllNVSS J155331+060143?ïX±ùëG?¼¡´b§?"ïÉ»›-5?¼¡´b§?îæ¿1rƒ?³'pŒX^(?¡ŸôXsÒ?³'pŒX^(?î¶&.?"XZµV?¤ž™°+1?"XZµV?ê^Ï$&61?ª>'Þ	mä?ƄÃog'=?ª>'Þ	mä?î
¶"´?°[š†X¾?¯T–%ãíº?°[š†X¾?ìÐÖl«?ÂïŠuþùŠ?¹!MvŽ#?ÂïŠuþùŠ?íÙâ¬T?§&›-!?·)0ëOŠ?§&›-!?åŸÞ€œ?¿ùF³b²?ÕÖÀCÚþÇ?¿ùF³b²AGN4FGL J1553.5-3118¿ï—Îåù@12—9m	À9Z—ü
¨À;ÃxØXò
@aÖ©?ý'RÛo&ÿ?«M—@+œÄ?µxs'-Â@
žÏc€@S¾	e"i?ïõäRûO—¿Àßȧú"¿ÞÚ/H¥5¿Û˜™ÿÅój¿àÑâœ'¿á`‰ƒœAGNbll3FGL J1553.5-31181RXS J155333.4-311841?ïýɸ?0oÈÌ× M?7÷P¬uĸ?0oÈÌ× M?ïЮ›ßD?…rUx{"?w¨²*zøþ?…rUx{"?ïâXbÓÆ?l;»~Ûý?më§Üe	²?l;»~Ûý?ïõp…½8?;¸¤þga?Uô¯ŽQS?;¸¤þga?ïü…Z%?5–çÒ>ò?;Õ-wg)­?5–çÒ>ò?î¶ÀŠ/†?´'(ŸÅþ^?¤"÷]ãî¤?´'(ŸÅþ^?ïÐå0yx?€~.»s™?wg¸E3??€~.»s™?ïáOòöF?Z8  »ú%?n°
4U!?Z8  »ú%AGN4FGL J1553.6+1257?ÎÇû !@Fš½çXÀ8àPšLGÀ;ÎtqÁä;@ïSpÁ@_æ\ÀË7?¨¿!œž6?¹ÏòF.®@
'âûã:Í@÷['¢Ú`¿Ú"
P»Ú6¿ãÖGj!ÜÊ¿â÷škP°ò¿çèŠÞ?æË¿êOP ,¿ïê=@RUAGNfsrq3FGL J1553.5+1256PKS 1551+130?ïù].âÊ?B˽ï®Ð?J‹EjŒg?B˽ï®Ð?ïóðÓ_y?c°·WĆÞ?XZüþ?c°·WĆÞ?ï·Hl3¥?€A¶½n›v?'-äè>¸?€A¶½n›v?ïÿ6ÈØ»1?:ÿÃÓ?&ã}R7?:ÿÃÓ?ïîKWõ½å?[Õ ñ¿?a´§ÞGá?[Õ ñ¿?ïÀßÒ¿?Ž
|äXå?Öã©l?Ž
|äXå?ïgù'§('?'h¦A°•?"Ï®Š‰µ?'h¦A°•?ïþ"‡…2?!¤ëCg?&ǐ€P²$?!¤ëCgAGN4FGL J1553.6-2422¿Û+
\q½T@6OÙÛ©¢À8²
RÎÙíÀ;Ëãktà @\ê«Úä¾@sÄóºw?§MìGŠ½?¯)PÂvm×@iÝcóÅ_@}ø¸¸îŸ¿»aX"Ì¿àڏbÞòi¿åL'jP¿ãGÉÃ-Ú¿è{ß@í±¿ä@Ï_~AGNfsrq3FGL J1553.3-2421PKS 1550-242?ïþE…ě?%HÍ͖­?+§¬XÍ!<?%HÍ͖­?ïìò@,t?p…ºø刞?cù
 7$¨?p…ºø刞?ïåVÌ?‰-?pÞ\û,Sj?j©3¿û?pÞ\û,Sj?ïþеºŒƒ?ÏÏñTsÇ?"ô¡óã³þ?ÏÏñTsÇ?ïù6dëçð?G"³QwùM?K&kà9Í?G"³QwùM?ïþe©°œ?•»)2ê"%?‹Àf™u?•»)2ê"%?ïµwépœu?'ÁPd=ä‰?'¢™â¾?'ÁPd=ä‰?ïýÎúpìI?&4iJð?1ˆ+I&¢`?&4iJðAGN4FGL J1554.4-1215?çÀ'ˆäs@>¨îÙ8À:­ÓÿÆõÀ<S'üžK°@!!šû™hò?ùÑ÷®ø¦?Ñ"ð½m?ۅlÜ!S@pŸ±@NoMjÁë¿ä3ÍêÙþ¿ï®3ïñ•?íé°"G'²¿±ìµàÍ	Þ¿âҊ¡"³¿åv_¢ýÆjAGNbcuGALEXASC J155432.61-121325.7?ïû¤dŽ#?C#ã«»]µ?Anpý÷?C#ã«»]µ?ïÂݟÓ_?†_ghq ?~'0S)Ô­?†_ghq ?ïG3u£E??Ž™æ^md?—'Foî(?Ž™æ^md?ïƒwá¸í?yZ^ï[,?"ŽU?yZ^ï[,?ïúðÅ0º?Ooöî	Ã?D<ë"VóÖ?Ooöî	Ã?ï.Ê <æ?¦%½ÐkÎì?š&§¦ÐùR?¦%½ÐkÎì?ï8ðž°|,?"3ÆqÎ?˜áì)ðz?"3ÆqÎ?îXòú!Þf?žiÛª¤ó"?ªpÐY––§?žiÛª¤ó"AGN4FGL J1554.9+2143¿Ë²Ý|6K/@H
uÍ·À:ºà¨KäÀ<'sϵq@ënºGäñ@Ât֐›?Ê<Kö"±†?ÑqP¥4@‡Š£\û@ó…mèÎ¿éòUóQ›Ô¿Þ¯ë¶pj¿Üž'¨'Y¿å×ï_ô²D¿æITrHù¿ïåXÿöoÞAGNbllTXS 1552+218?ïé¢ôU?g5k%¾Î?f]
¨b#?g5k%¾Î?ïà…w‰àz?t>㚸‹I?ozˆ˜{–?t>㚸‹I?ï¤zô›{z?ª:»7°
?†áBÕ±…›?ª:»7°
?ïž[éÆéÅ?i¦½%\•?ˆi˜"b­?i¦½%\•?ïÔ=ÔÌË?uþŒ;¥Ü?uõa6•Ú?uþŒ;¥Ü?ïIÈ®Zÿ?¦ï‰
6W?–Æê8,<*?¦ï‰
6W?îiœvõ!?@!ô••]?©f?Ùl"ê?@!ô••]?í¹U°ä(?˜´rŽ7?²5Wœ÷Ã?˜´rŽ7AGN4FGL J1555.2-4149¿íÔf³U@"
?·¥ôÀ9eR1%;úÀ;rƒ]œ"@š–pÅ:@eÐÄ©Ý?ºB÷ ˆ`·?ÈÏÒ»¤0v@üÿý@öQ'S?ïß¹£ûk¿ãâÑñÏ»•¿ç†‹À)M¿ç|ŸÃF1¿ç:hŠ'¿¿ïüÇ0«™vAGNbcuPMN J1555-4150?ïæH-3Û?fI®Ö´Û~?i·Ó"Gĸ?fI®Ö´Û~?ïÅþ'?Šìb‹²ÈŒ?}w|Y³ø°?Šìb‹²ÈŒ?ï§èÿTÖ¾?~aAAËrÌ?†À#ër?~aAAËrÌ?ïí^ZÜÍÿ?Gº2˅›˜?b¡¥7Ϩ‰?Gº2˅›˜?ïâ*Fûg?mBQŒLB'?mÕ¸ÞL*?mBQŒLB'?î
ïyAÍ?¼'õËɗŽ?¯!mŸ±/?¼'õËɗŽ?í¦"Ù:Â? ËF·_ØL?²ËÙ7uTn? ËF·_ØL?ïmTðOçR?«HÖ!!?'Ua÷ºãË?«HÖ!!AGN4FGL J1555.7+1111¿ïã¶"2Ò2@Eû~|âÀ6{Ãiv¼À:xßN¯|@üØ®,x¯?ø¨–<"?Ž¡öVÖGí?±cXÊÇd@¯b_p¨à@²‡ªƒÌ©?Ù͵à¢Á¿Íù2±-4¿Ö3=ú·k½¿ÐHÏÃL¿ÙQºÀ/Û¿Ù.šG>'óAGNBLL3FGL J1555.7+1111PG 1553+113?ïšFf'?¯{?2E?‰n{pª0A?¯{?2E?îý&D}?³[è GEª? /=ž/Ñ5?³[è GEª?ìnÍ[Ï?©x!ĈÌ?¼	•!‡1?©x!ĈÌ?î<*²}Ž?—8 :¯"³?¬?XGÃ"?—8 :¯"³?ŸîXŸ?š,‰wþã?ýŠ Q?š,‰wþã?ëdŽ)ÎÛp?ÊKpæ5î=?ÂmÇXĒA?ÊKpæ5î=?î´@ø©Û—? @C(]V?¤»ðrΑ? @C(]V?èµùR"ò?¹^Ï2?Í(·wŒ:?¹^Ï2AGN4FGL J1557.5-7040¿ïáÈEî:ŸÀ*Odñ`¯À9¤Ãð…8ºÀ</)¹6íÓ@ąrp4ñ@ƪ#T˜ß?³îÅ`ß$?±7Ä<…lf?ýQ‰)ßÍ[@Ž88€¥?ïëÿ,›i}?Öwz?·%¿äV4ŸÄÖß¿Þ»#­Y¿ä5YžVí£¿ænC?ñCAGNbll3FGL J1557.4-7040PKS 1552-705?ï÷¶šRÉs?DJ#"KŠ>?P'Ëœe™¿?DJ#"KŠ>?ï½?3¶??‰hµz¥×?€°3/sˆR?‰hµz¥×?ïÙ+‡î …?qŽrüŠ?sj;ó¢)Û?qŽrüŠ?ï/W|FU-?'r3j
îÅ?šsžs?'r3j
îÅ?ïß^@8eˆ?eÛ\e9HT?pPßãOÖ?eÛ\e9HT?ï_ñ2V?šó²§£Æ?"Áޑƒ;?šó²§£Æ?ãbv©?‡€%è'a?‡‡5 Å´?‡€%è'a?ìSÍ:8"£?§+2U41W?½a–.;bé?§+2U41WAGN4FGL J1557.9-0001¿ïƒ2–øvì@BÔÝÖàLÀ:®]Ywj›À<3nUH0ñ@¾x,a‡Ú@ŽÉ¹òÕu?ÑÆláTÄ(?Ê5öHÇ?õ.éÝ~˸@hØë>'¿äùn‡P¿äÏ© ø³…¿áNƒ†1ÝÉ¿ä­¡ŽZ¡6¿î´²ú"¯¿ðAGNfsrqPKS 1555+001?ï˖‡I¡?vS(Aœ"?z4¼|rïB?vS(Aœ"?ïêx`Ü09?p½Ú­ìP?e‡žòUfÊ?p½Ú­ìP?ªF)?Œ5žk'*?žéèÿlä?Œ5žk'*?ï×)žC?ZëV‹Œ"?tk0ù½³º?ZëV‹Œ"?ï«H"Âá«?†¢t¡??…-ÞÏG•/?†¢t¡??ïy|T~ [?™`Î:ÏÎy?ÐukŠ¡?™`Î:ÏÎy?íãã"_âz?¡Ôº_{ª?°àæë·²?¡Ôº_{ª?ï:§|—fu?…M|¦ù²?˜«uª7]?…M|¦ù²AGN4FGL J1557.9-1404¿ª"pmzâ@<Îü›ÇqCÀ;ä܎
ðÀ<¥³7ÐPæ@ë%ŠÔù@U—Ià?Ò)õ1oä"?èQ¤7'M@›ß°Õ @¥õ¢"?ïèçë6D`¿Ï¨ýz>µr¿ÆQˆöÄm¿éprž®"¿íTÝ!®¦q¿ïþÛrýœAGNfsrqPKS 1555-140?îZêê¡Û?±­j-ô™•?ªQQ]>P?±­j-ô™•?íi×+—Ö?¸e5b›'O?·ô±D}Õ?¸e5b›'O?ìܱêø?£C±b(¸?¹ây'½?£C±b(¸?ëNÏYM?£­ÃnÀ'0?ÂÅËÄšÍ?£­ÃnÀ'0?é/Lú¼£?ÅקèÍ3?ËBÌñ
t?ÅקèÍ3?åÈËRp²'?ÏDƒÛ?Ôni[šÜ?ÏDƒÛ?åaqK¿œ?»¼åÎü?Õ=hÚÇ?»¼åÎü?ÛÖ'´¤âÎ?¹LmÛ&Œ?âì%­Ž™?¹LmÛ&ŒMIXED4FGL J1558.8+5625?íÓ Y.øï@Fá«\9¼ºÀ99¿×hÀ<J໗@Ÿy•în@iåŸ+©Ò?¬þ¿õ40?­$g_×ùH?ýFÈ •¡½@Úœ&g?ïÌÔÉ'¿äÒ`v¸C¿áÃq~óP¿Ý$O\^¦¿ãwomv% ¿ïÿòß0&¹AGNbll3FGL J1558.9+5625TXS 1557+565?ïý¯BDÀq?$°ÖYŸ‡m?2…ëã'i"?$°ÖYŸ‡m?ïöl,ñG"?SË텨@¾?S'¥ùµÌH?SË텨@¾?ïä/"Òã?x~³›ï¦i?kÐ{þ¦¸?x~³›ï¦i?ïìçû/q?Qdu+Ó?c"–Ö?Qdu+Ó?ïý\‹Šüã?1+oœ$vG?5¡ÂûW?1+oœ$vG?ïØ+Ò/¦û?u'¹ì_?sêõêò5?u'¹ì_?ïäåJ-Þ?xOymßÁn?kµ÷ñÜ?xOymßÁn?ïàÓ	ÛS¬?`*Rä|_ƒ?o,õås"?`*Rä|_ƒAGN4FGL J1558.9-6432?áylÿÜÀ!F‹;26À8©1½nÀ;ÒêVJp@²X>…vÍ?ÿA9k[˜­?¤âb¶-¤?—Wºã&'?ñ²žÓ•=ê@פ"G ?ïíH"-§X¿Ù	ÿ}y'‰¿àS™Û¿ÞSCο஗WŸú¿×uq{î8AGNbll3FGL J1558.9-6432PMN J1558-6432?ïý<aQÉ?,.áú²?6ù,˓Ó?,.áú²?ï綜2a?tÅ嶝?hIú|ŠÎ{?tÅ嶝?ïÓ¾i:^Ô?Nvý,Ò?v Ë{ÅÉ?Nvý,Ò?ïÕÝÿŽ?e…ðàsË?urø©Í)?e…ðàsË?ïò
F­?W!ŠÖ"Ž'?[åsÔçb?W!ŠÖ"Ž'?ï˜D®A¹?š-Ví{Ï?‰îÔ}~¤?š-Ví{Ï?ïÊï[(Uñ?"HÂÌKÓ'?zˆR‹qoz?"HÂÌKÓ'?ï˜ÀÙØ»?~(Tšz'?‰Ïɍom5?~(Tšz'AGN4FGL J1559.1+6736?å""èe7E@DcEŒÒ
úÀ:ö*rDÀ<á‰$@›½Ñb^?ý…‹ûKeY?ŝ^J82v?Â3Eèª;?ú®ç¸5f@M¥ÿX¿Ú(ç	D¿ê¡uÁ"I¬¿ÂA…±ZV¿ä mòKâ¿ÖV>{ë°¿âž8ÀúõAGNbcuNVSS J155856+673646?ïþ˜~çf¬?[Rê°à÷?&xºU|?[Rê°à÷?ïõŒâ&%Y?W†û[ÿMß?Tæ;8_X?W†û[ÿMß?ïó
áQál?SNÓSªm?Yê=à.(/?SNÓSªm?ïó'ñô=n?<{·¹¾íÿ?XÜ(D"?<{·¹¾íÿ?ïø´NH.å?LÖ úå
?M.Ç×ÁÃL?LÖ úå
?ïØ*
šP?w˜0aì_?sêù=°?w˜0aì_?ïäªZöµm?t,P$4"˜?kU¥è:•?t,P$4"˜?ïÑñ7¡=?c҂J5?wvÌÒ	"?c҂J5AGN4FGL J1559.8-2525¿åô(Ì@4'"àÞÓÀ:^ם
gbÀ<#¤¦©M@éш'›@r=Ÿ¿™?¾húÀP¿ˆ(ÎÓO?ÉÏa<0@|ža)'¿ã_¿"å­¿Åÿ{&<¿çL_ß¹Ž'¿æü¿ÔKK'àD¤¿ìSŸÍ:[AGNbcu3FGL J1559.8-2525NVSS J160005-252439?ïü¶Ní4?:× P!"??êN^ãm?:× P!"?ïê¨×mæ?wáê/ÒL?eWíôX
½?wáê/ÒL?ïéô·3w?[¯u5¥–
?fü6îÙ?[¯u5¥–
?ïý¨hO°Ô?â—ÐóÎE?2¼¾±ð{Û?â—ÐóÎE?ïó6ƒ9ä?Tý'ê¼`?Y"îÿ—C?Tý'ê¼`?ïƒE•òN? Ïºù÷¹q?.š'Œ? Ïºù÷¹q?ïÐó¸ýj­?}Åèô?w†#iíQ£?}Åèô?ïòé£aq?P™,Û®þ?Z,¸ûøŸ?P™,Û®þAGN4FGL J1559.9+2319?âžPøø­@G¹I¾ó(À9ßÛz¹×À<<¤:Œ@7'&«;@^ÁVw?³dŠn-…?q½
«Óò ?¾
~BÑ
õ@
æéI?ê§Tm@?Ý¥h"αS¿åŸÁ}ä1¿ä3aÁ»÷'¿×áËÌòŒz¿íÙ®'O"}AGNbll3FGL J1559.9+231987GB 155744.0+232525?ïü³Àó`ñ?.ë5k¢?:aø«Vڗ?.ë5k¢?ïõUÂ@þ?]Ö'Ñ?¢&?UT{…o±?]Ö'Ñ?¢&?ïçLŒ(J?kzB^ç?hî³N»í´?kzB^ç?ïôD 6?EÖYY]Íd?Ww¿ft3?EÖYY]Íd?ïô!|i
?Pc«3ñ?W½/ã–=?Pc«3ñ?ïÐÂÓNÇ
?'ƒokÌ<?wž–P]iS?'ƒokÌ<?ïÆhtˆ"?'µõ ô?|ËŬ˜2?'µõ ô?ïæS_^Æp?\Ze]D,>?i¬ f H/?\Ze]D,>AGN4FGL J1600.0+8510?ëD7ÒK´+@>Z_¦XĽÀ:š""œÛÀ<Š4 ˜ü¼@tÊUú˜@bÑ6¿?µÞj(ÿS?¢¤Á¦?ë•ÏªÍž"@9"í];¿ÚÜÒČ¿ãÓșae¿áÚ¢þ)q¿ÞacÝu¿áŸÑâ5iÄ¿ìÔUøZQAGNbcu3FGL J1559.7+8512WN B1609.6+8517?ïü;Ü
h ?0vOP¸?>!ŽÛ'w?0vOP¸?ïôÕ_Ëö?WÛ҃Úè\?VU@RT?WÛ҃Úè\?ïó¤Ý
?`ê°xÞW?X¶E–t
"?`ê°xÞW?ïä7[¥±ð?TDé«`.ª?kȤeLÐ[?TDé«`.ª?ï÷ôpȕ?EAoT2!d?Pû)· ?EAoT2!d?ïӱƔ¬þ?|šVÌ5?v'Ïœ°?|šVÌ5?ïéòG/¿`?wA™MO†T?f
¹øÏN?wA™MO†T?礪—ÑdÙ?rß)GL?†^™ýèY¸?rß)GLAGN4FGL J1600.3-5811?â:¤"}¾Àœ¾|§ñKÀ9²~'ÖV¹À;³lsÆ¡:@$-"$@©öùÇÛ?¹H'OÐø«?Åz‹vì›@
IˆÅ5ÿ–?ñ˿ɯ?ïýqz–Ÿ?á`·Ð¼E–¿är4ÐÂ$Ó¿á™«ßí;¿çO ~ûˆ¢¿é(ž[ÙAGNbll3FGL J1600.3-5810MRC 1556-580?îù@qîž?¯ìLK¶vo? køï¼ý&?¯ìLK¶vo?ÞLP¿ÏÓ?̃5ÛÈØ?àÙ× €?̃5ÛÈØ?îºzÝ
Y?Ÿû[ÙÚ!U?®DXR/*n?Ÿû[ÙÚ!U?ã͇´X¦y?°lÄÆ»]?Ødð—N³?°lÄÆ»]?ê{6d–µ?Â7Ÿv®?Æ&m§ù.?Â7Ÿv®?¸¯C"º"?ÂQ "€GZ?ìꏭv_?ÂQ "€GZ?èL—¿Ç?³qT°¸Br?ÎÏ·Å¡ã?³qT°¸Br?¸ïހXžà? ×ÖÔ¬õ?ìâ/Ë°Ô? ×ÖÔ¬õMIXED4FGL J1602.0-0641¿èð˜‰NGâ@@lÚãæÄÆÀ:ÃÌ­ÃJÀ<J¶¶^Ì@\ÕOÓ'@p̆Uï÷?Ïz4y"P\?Ò_Û\Ý{œ@×z€ÎÇ?ñ"icñÁú?ê¬aBD?íAd®L¯¿á-¹v®³¿âñ.«äö¿é–}_Ò"¢¿ïþ¢NZAGNbcuNVSS J160146-064256?ëmÕî´~!?ǐïö/û?ÂH¨E.z?ǐïö/û?â®}sô–?Ѐä«šV?Ú£ÎÔ?Ѐä«šV?í

?ê¸?£^½€¢©m?·§—•$ÃC?£^½€¢©m?á³Ö¥Ø[?´''ñç'h?ܘR´OIâ?´''ñç'h?êëXjËP?ÃÇ®|]?ÄRŸªTÒÀ?ÃÇ®|]?Äöä½F?È4c:s)ª?êÿÂFи®?È4c:s)ª?ê]ø">F?«åÄ.l®?ƉÈïç?«åÄ.l®?éío?°3ã
Â:—?ëzœ"¤??°3ã
Â:—MIXED4FGL J1602.1+3324¿îÌþy×Ý@HZõÊÀ:ŽFipÜâÀ<¨´ú¬@×	µ5l@k¤"ÈŸA?Á8ø²<(?¾â_&ù?û‹­b¤:@~ôþð
•?ï¥^^Z(k¿¢ÃÂbÀ¿å¯Ö(ôì¿ábòsO'õ¿çÌÀ7"D¿ïõµ>:Î2AGNbcuOS 300?ï÷O†"Èé?OcüD'?Q`òÀp­Æ?OcüD'?ïڕ¾©Ú–?sqHßLZ?rµ ºàé?sqHßLZ?ïٟÿ—ØØ?w6qŸ^8?s04À?w6qŸ^8?ï>IWÈúì?x¨"yI¾u?˜6Õ¹8|?x¨"yI¾u?ï–}V(;ð?•õª?Š`ªƒ¯t
?•õª?ïp˜àGd)?˜exÉ£>?'ìãó£Þé?˜exÉ£>?ïMªÙpÓ?•È3"ˆæ÷?–J¾ýò­´?•È3"ˆæ÷?ìμ#Ú²?  kM‰~L?¹Šå¦ëð?  kM‰~LAGN4FGL J1602.2+3051?í?^ÓR«|@H5Þ½çÀ;¹†žëÀ<¼}ÄY@×kÖïí@mç˜ã?ÄÅd"¿H¿¢ã	'¾>r?ý/|&ìþÆ?ïîýy=¿æÊ?d‡¿á5tV2¿ã0‰4LJé¿ÔZe]Që¿ðAGNbllRGB J1602+308?ïñ^9ú«5?UºÉ64°d?]CŒ(õø?UºÉ64°d?ïðC|…Ò?n^1X?_yüô\ß?n^1X?ïÍ{ç²h?u=˜¨2,±?yB?Ö¸>?u=˜¨2,±?ïá`öi?TŠÊê?nŸ	ã1&ä?TŠÊê?ïÉ*D»à…?s	ÐnY\?{jݳ=ÉS?s	ÐnY\?ïć{VYö?ƒbêi•?}¼B^qì×?ƒbêi•?ï•Èçdþ‡?ŠM–ëý/9?ŠÆ4~Î?ŠM–ëý/9?ï^Yyg?"5²÷\?"4ß4ø=?"5²÷\AGN4FGL J1602.9-1928?ÙújÞßãš@8C(ÃnÀ:5s"u"*À<([{PÙ6@<MŠ!…@\ޅ[ôó?Òõ»ƒyG?µp$À©¨Û?ò¢êÊ
Ö@ŒrêƒA¿²#½tj5(¿ã6 M}aU¿á4DZ°è¿Ú"UÅYeø¿æTÞÿQš¿éUõÀa¦AGNbcu3FGL J1602.8-1924PMN J1602-1929?ïþoà@O¯?¸
åþçµ?)þвŒé?¸
åþçµ?ïêÆY/
?q¯)‹°?e9¦ú12H?q¯)‹°?ï÷ÞݵA/?Gwn1;?PBD³º2f?Gwn1;?ï÷æ•×~?3g‡œk®î?P3ò™7»'?3g‡œk®î?ïþÇB–Ÿá?‹'¬«ÙI?#‹×…³s•?‹'¬«ÙI?ïÿô¹È0?œÒ"åÌt?ŒÃτ)?œÒ"åÌt?ïöÏñ_~?cðRIä#¥?RaâˆtÒì?cðRIä#¥?ïâTûæ@?X7o<´?m«oF?¿?X7o<´AGN4FGL J1603.5-7112¿ïßåä~wÞÀ+đ)ˆ†À:¼ÿc"HÀ<3`:Ó:¥@*Ÿ"ƒªð@û¯S?B5?ËÉB	9å?¹¾'ø?Â8?ñkŠ'•™Z@¯ËE¥Q?ïü	 ?
¿èâÒþ?5 ¿çE^í{Ä¿à–±RF¿êtjÀ¾ ¸¿ïþ°à<4AGNbcuPMN J1605-7112?ïò	½n
?^u·X/»?[ì…vbb?^u·X/»?ïÜ!¨é?x"²‰'0?qï+šV8·?x"²‰'0?ïÃLíˆGü?y›êÜÎy?~Y‰Kª5¼?y›êÜÎy?ïÑø—ù'ì?V6¨ìï?w³äŽ.?V6¨ìï?ïîÖ:<o{?Z­U¸j&|?a)Å¢"E™?Z­U¸j&|?ïšã¢•÷?"åu¾‡µx?‰Gof?"åu¾‡µx?ïˆ?í¤?‹ÛJt…?ð;¯'?‹ÛJt…?î§t0BW?Œ>{Fåp?¥Žø¼ûړ?Œ>{FåpAGN4FGL J1603.8+1104¿á+t‹JÔî@Eü'œýÒÀ:¤Z7ƒúÌÀ<Kü²m¥ö@ñ< e'@ð?)á{?Áà;êf政U³·µµðB?™¥Zˆ.@‡hÆ=­¿ïž5_³Cå?ï´øÐ`ֿ暉ÿÖ%¿á%ÀN9H÷¿Ù°L£òý¿èò5ÂY¬DAGNbll3FGL J1603.7+1106MG1 J160340+1106?ïüf›ž	I?1Û!ck˜?<Ë#µ¼t}?1Û!ck˜?ïòÒé؇|?aAh3³?ZZ,±åÆé?aAh3³?ïí-Ú¦ ³?\Jbá‹õ'?bÒ%‰ùÔÈ?\Jbá‹õ'?ïó[nˆZ?AͬÐȬ¢?YI"‡a,D?AͬÐȬ¢?ïî,{犜?[¹ÿÐq?aӄ"L?[¹ÿÐq?ïµÑð<}?Š§³/TÈ?'‹ƒù>°Ã?Š§³/TÈ?ïڈã¡O?x•Úgš?r»Ž"+˜l?x•Úgš?ïíu{?q)íC¢²–?~r)X·þ¿?q)íC¢²–AGN4FGL J1603.8+5009¿ïî0wõ"@Gz·ÃPLIÀ: ÌìÀ<§P;¶N@ ,¸¢v³?ûØ	@ñaØ?Âø'6H¼\?Æ1‰Û@ƒÛÂ3?üúWŒ®ÏŒ?鸊à刺Ð8Éà‰B4¿ÅPäÉî¡¿Ûü'œýÒ(¿âK"é\P¿à¿p\‰nAGNbllSDSS J160339.49+500955.5?ïõM*ï܋?Q¢©ÎF$Í?Ue©ãÍÊ?Q¢©ÎF$Í?F{dz?Œrõý¬?Œ^®]·Ep?Œrõý¬?ïÛFΒí?sòØYݾÐ?r~ܜ&%~?sòØYݾÐ?îXb€äÓ?'úûRe¢?ª™Ô'Ô?'úûRe¢?ï°møoט?€®µàw#£?ƒäçÑ«ô?€®µàw#£?íªĨ?ºc'>º£?²¯M°Ãôå?ºc'>º£?6G9Ð?8\ÞP£?Žrq¡'ä?8\ÞP£?éç!A·%?§¼`õ·r`?ÈczûÁ#n?§¼`õ·r`AGN4FGL J1603.8-4903?åK,ñr@›†»ÒªÀ7¶Í׎ǮÀ:¹oó­â&@ 4ÞÁÁÖÐ?þ'ü\'?£Ê`0žj?¯Ab\&ؘ@ŸÆ¤"Ÿ_@ô<ö*"(?ï±ÃŸ|Ý¿ãC´VÝ\¿áŸÆ¿l'ú¿ÚÜéåâGˆ¿à…_L–²¿ßt¤9/ÌAGNbll3FGL J1603.9-4903PMN J1603-4904?ïøGâ Q?QÙAhÂÅ?O'àÆÛàÄ?QÙAhÂÅ?ïՋ•Óo?­5ñ4™?u:5#Wð?­5ñ4™?î'äØ"Ø? ±Žì›?¦Ñ²'Ò5u? ±Žì›?ïÿ,æ'ñŠ?`šã\?c'Æé	?`šã\?ï÷6'G̯?QƒTjÞ÷?Q'Ý÷RE?QƒTjÞ÷?î\Q°Ty²?¸pqÌôè?ª:äÿçÒ?¸pqÌôè?ïþñÚoÅ?%B‹"? !ÁBke?%B‹"?ïþÑfågM?¶KW"7?"é"6§L?¶KW"7AGN4FGL J1604.5-4441¿árÓÚ¡æ@­§m˜À8ŸïŽ˜´—À;Žh
/"@_«Jqg@Ez]"?­NÀàãã?µÔšaÂÛ@©ŸâÚU@ÿ]®1S?ïéÌ¢Zˆb¿Ûf&ºÿÅÈ¿æ'f pbê¿âééþ‹á ¿ì,Þ_Ç;¿Ó5nA&:ýAGNbll3FGL J1604.4-4442PMN J1604-4441?ï¸_x>2É?±t‹C‡Â–?è"A?±t‹C‡Â–?ï×0'G?QcÈmì¾?tgþ›"€?QcÈmì¾?îF"à'8? Y[Ϫ9ß?«–ÎN‡@‰? Y[Ϫ9ß?ïýÆI¥æY? I/‹"®˜?1ͳ¸ÌoØ? I/‹"®˜?ïÆ-CZ×?zËÄuL?|é^rüV?zËÄuL?î]¸]cf?·r[ؑþ¥?ª$vý™e›?·r[ؑþ¥?íïwú	ò?¡ÕŒŸA@–?°"@.•Õð?¡ÕŒŸA@–?ïø'#A‰É?BêáÂ˕?M÷rxΛ?BêáÂ˕AGN4FGL J1604.6+5714?îŒÁøï{µ@F^4\þޘÀ8¤§.­'uÀ<Õº²@±ÔÎÎÛ@ɐ¢zì? u ŠÜ_?³……žÙt@²¯CO
)@7cI¿×Qaz>¿á¤€-ŒÖ¿æ|fîK¢–¿ä/¥²óˆ¿í•ao0º¿ïÿ "_õAGNfsrq3FGL J1604.6+5714GB6 J1604+5714?ïíàRæÕ?\{Ìl'6?b­kc?\{Ìl'6?ï鑓ˆ)ý?uƒÏ†ÿ Ò?fnlÓ'ë?uƒÏ†ÿ Ò?ïrZª4`?‡ü°GäxÄ?Œ#i\Rä?‡ü°GäxÄ?ïÒ(S'¼ª?ch5Îäï?vëÖUt?/?ch5Îäï?ïøóUïî?B£üPÔ?L2¨0V'ø?B£üPÔ?ï«îþrt?ª9½Ãã¦?…@r+?ª9½Ãã¦?ïÓùä:°?'†8}oÎ?vr`ÇÐ?'†8}oÎ?ï&4?‹¿…riŸ?›>ƒ$£~?‹¿…riŸAGN4FGL J1604.7+1734?ïĀü¥éš@FICä/À;(2Æü©3À<£Ø涂Þ@h˜ð§H?ý¨PKqîZ?ÖxŽ·«?ÓÈxª5É@ÖV%¦'¶@üçõG?Z¿ïþ²Þ=°?ïÿ
×ÊVÑ¿Ú%¬!†x¿Ö<« —¿ì¦>Ê.¿ï÷Ÿ¾÷¢AGNbllNVSS J160436+173324?ÎA¨'?ˆ)[AdçE?‡žÌyäÊ$?ˆ)[AdçE?ï(ý¨óåÒ?±¼gèC6;?šàJã;Ë?±¼gèC6;?î?š"$ò?˜k7À!?¬öZ=Lâ?˜k7À!?î~¥×vF?‰¢A¿Û%??¨¢‹}§?‰¢A¿Û%??îþHìò á?›Û+Ð1? q.B<ù?›Û+Ð1?íƒÞ~Ðëj?½î¹=›8x?³á	
±-?½î¹=›8x?í¸Yα%?¡õssoW?²=1ŠwÎÕ?¡õssoW?é˜åš©–?µI•î'>?ɜi•ùY¦?µI•î'>AGN4FGL J1604.9-3414¿ïðÙB7CI@*Û=ŽcÀ;D@\çbÀ<}Rkî@!…çïf?ü-Yvɋ?ØÔ Ö¤¼ã?¼'	AóŠ?ì"D¶v$@½_&V+?ÁóAÁ‰?ïÿ§¬_o¿Þ'{%ì¿Ø~¢u¿Ó$¹½üOq¿æ?,î‡ÞAGNbcu1RXS J160452.5-341407?ïþ¥i¢í? µ‰I_÷?%¯×'1–? µ‰I_÷?ïÛì(Bûc?~"í~rh?r	ëÇÔâe?~"í~rh?ïîuÚUT#?k}¨_J·`?aŠ%݆Ä?k}¨_J·`?ïúVº:½°?3•bìÄ:+?F¥m‹ü±?3•bìÄ:+?ïÿ@(j?cg°Kþ?ûe0°š?cg°Kþ?î©F&nÃq?²£¤@ƒ×?¥k™ï¯ð?²£¤@ƒ×?ïîµÈNbä?rx]SW?aJ7å×+<?rx]SW?ïê¥øo	p?Z072JÅÁ?eZÐ/`?Z072JÅÁAGN4FGL J1605.1-1140¿Çûøߋ}@=½ƒƒ­ŸÀ:U%t9ŽÀ<,=CWm¥@ 
ä‡(¨Á?þ'Ï…ä°ï?Ç7y©d<ë?È£}É@-gAW¹$?ýîGSP´ù¿ì!"Þ™¨Þ¿¤öw@(d"¿ÏDYKK¿â:¹ÚÁ6¿ÞCùÿàË\¿ïÿy\ã/æAGNbcuTXS 1602-115?ïùktJÞ(?IwoŽñð?JR/uÑ?IwoŽñð?ï£68v>??_#l?‡;r|1Dj??_#l?ï¹óøúl?|ô{S'?ƒÏÓZb?|ô{S'?ï¡°
,?k¢[\a±?‡¹T"2r?k¢[\a±?ïô[W?cȋP&ó-?WIÎ.‰ü?cȋP&ó-?îV>džK?´¨*ãbÎG?ªœFFN?´¨*ãbÎG?îpà§9?¹ÉÞÝzØ?¨öñòøºÏ?¹ÉÞÝzØ?í¢'ÿm'?¡D-.÷P?²ëoÞÑ÷?¡D-.÷PAGN4FGL J1605.5+5423¿í@¨¬‡@FƬ![š[À;;¡…÷%À<ém ‹]@ ˆ"Té'T?ú²ÜÌQ$?ËÛTyÿËR?ÇڇËeï?ýšR[íf @ò<˜Œ©F¿ïÿž`¨·D?ïß½4©Tø¿Á0Q"Ñ¿Ó^¢!Ód¿Ý.¿»Â8t¿éÃf½Ë¨AGNbllRBS 1555?ïü#Z*Ìe?4ø·‰šL?>å,úš§G?4ø·‰šL?ïå~Uà +?mÑêÑ?,L?j©þ㕧?mÑêÑ?,L?ïçš{õL{?a•J¢?he" ±€?a•J¢?ïÆ< Õ^?^ÄÆË+d?|áþ΁̬?^ÄÆË+d?ïö£y±
¾?OBeƕØã?R¹
ÜÂæ?OBeƕØã?ï©ÜN?'Õ"sN|?…¿ˆóWpÂ?'Õ"sN|?ïϓ=Vo?{èË?âά?x6a5,<?{èË?âά?ï=»ÜÜܲ?ƒ³á…ÌÌ7?˜H"_<ÿÏ?ƒ³á…ÌÌ7AGN4FGL J1605.8+7208?åno87 @Bõ¢ß"xîÀ;â©,´"ñÀ=2OŠÎ¢@!LçÂFŒ?öX¡fítã?×
£|ÇPâ?ÕÁ—Å.ô?ö
e´¿@_°
tM/?ïü¬ž"¿Ñì"xK¿î"'r4Ñ?ä𒤲ÒP¿åÖ<b0÷š¿ÁÕ;ƪžÐAGNbcuRX J1605.4+7208?ïñ"È#šº?`=#Ä¥?\ÖoõC¬?`=#Ä¥?ïôVæ/Ž'?U	ÄvÕZù?WR3F.·?U	ÄvÕZù?ï`¬gãa?f¸½Ç?"ê}l$[ù?f¸½Ç?ïì(·wŒ?Qy
í»g?c×åh$ۚ?Qy
í»g?ïâ§V'¼?r¹¥ÓŽ²á?mXð³+?r¹¥ÓŽ²á?ïÐÆAwk?|e˜Â}ï?wœß'Ðî_?|e˜Â}ï?ï‡e·¿Ê[?ŒYÉEEê?Ž&'þß]b?ŒYÉEEê?ïŒ	Á¨_?u€"Î?~¹ûï@¤?u€"ÎAGN4FGL J1606.2+1346?¯¾ÓdìhÉ@Eac^t)žÀ;]™J¿@óÀ<¥äŸQi@"j‰¶¢"?ûG'Æ}¥?Íkè.R#?©ZÞB ?ß³ 9†^@ÌR(–Í¿ïíû@R«t?ïûA
r¿ÛÙÒ#£É?¬öoÞ_Fb¿é2ŸÅ,Å[?нw¤ý%AGNbllMG1 J160619+1345?ïý5BF?5õ±úZ
.?7çÄ?ú(?5õ±úZ
.?ïïÀIܗñ?h¯[ÇÙÍ?`?µð×O?h¯[ÇÙÍ?ïϺ1-ŽG?s¹	 	™¶?x"çOÔl?s¹	 	™¶?ïê£Ú»"?PK±ß=?e\%F=Øz?PK±ß=?ïúÑ$(?AÁÄÏwmT?F»÷*­?AÁÄÏwmT?ï®Qh
Á›?;±rE{?"k¥õuV?;±rE{?ï¥a:s"?‡Î@æJE?†§±ƒqïD?‡Î@æJE?ï±×y+Æ?z•"#†ç?ƒŠ!µŠ?z•"#†çAGN4FGL J1606.3+5629?æ|vh‰y@Fbb#ᆘÀ;&,ºs.À<Îò`Û+@!"5Á­ßÍ?ûvmÊÞ¶?Æҙ•gÛ±?²;-}'¦?ếBŠ¿@}ã¾V¿ï¯IÏVêÈ?ïìá?J˜«¿à‡Ëp¬:†¿ÝɨÀ~	ñ¿Ã<òϕÔé¿ÞÌDý
,TAGNbll3FGL J1606.1+5630RBS 1558?ïÿ\í'?ݘ_õÿ?_x¥IØ?ݘ_õÿ?ïõÓ¼ÄÜ?Y.6L#?UæXÃE?Y.6L#?ïõrqGÒ
?T®ùKD^?U÷i¦à?T®ùKD^?ïùG½a}|?4¹`ÌX?Já
ȧ…Ð?4¹`ÌX?ïþCr¤œ?#Dª	¡AË?+ÈßÄòäV?#Dª	¡AË?ïÕ9§ãÖ¡?u§L'!?uc,ě}?u§L'!?ïóŸo–´?fqÆôøS?XÁ"OƒF?fqÆôøS?ïæèvj›?_Wr²kùÖ?i‰×Ø55?_Wr²kùÖAGN4FGL J1606.5+2717?ä…Ö£æ#¶@Gs¹8›RÀ:"¾³.–À<iÉØü…ø@
ÿ¸\}@¥Áƍ?¿)âýeÇ¿´{ç¾%ü$?ô05½Q.Ç@ÔL\$8¿Ô< A¿¿ç×ä'‹¿æ"[t›¿ã"8^kEH¿ç0=µm5¿å9̪hAGNfsrqB2 1604+27?ïý‹ˆ"¾?+ځ ‹7è?3"£è² K?+ځ ‹7è?ïðÅã#¦M?brûÒù&'?^t9?Á%ð?brûÒù&'?ï␤¹™z?u#—jÝqõ?mo[/	-ª?u#—jÝqõ?ïíÀ-¾:t?HJKªö1?b?Ò
Ü@?HJKªö1?ïûW
—¢b?BN¹ÛAäö?B£Ö
ÿœ?BN¹ÛAäö?ïÁO	lT+?…9'ðH'?X{>×*›?…9'ðH'?ï̕s³ð¢?W[íœ:?yµF9E?W[íœ:?ïHvoæ?…gSæ—ð?–ñ>ó»?…gSæ—ðAGN4FGL J1606.6+1324?Ü>PJù¬@EB¹¡vÝ­À:â°"rÐÀ<OŠë€í@+^a_@'@ô	¢@1H?Ï,—Õõ?Ã,éØvN;?ò œÃÆ@RÐL^'~?í¥"à¿ÙSº|¾§¿æ¹þúFƒ¿âBH§µç¿ê$«°óR¿ïÿI¤ë‡AGNbcuNVSS J160654+131934?ïåސ»ñÖ?eГüÚ°2?j!omIz5?eГüÚ°2?ïÙӃJLÕ?{'q`ÐÝK?s>h˜J?{'q`ÐÝK?ïŽ7a|Wû?"(ÛdîØÂ?Œr'«8Õ?"(ÛdîØÂ?ïxЩj?p «Õ[¸?ÿÅïú(š?p «Õ[¸?ïfÄ>g´?©žÃC?"'"Ÿ–?©žÃC?ïûZ&?§p°v(?œÀ7µƒB?§p°v(?îL¤Q=ÿ?ŸÕ±!ötç?«5ºïL ?ŸÕ±!ötç?ìÐ+‡Ô[s? "÷,Ÿ‹?¹~£Â9j? "÷,Ÿ‹AGN4FGL J1606.9+5919¿î¯Û5¬pr@EÙßeUÅÀ;X)º
­hÀ=qÞ@‡qÎÏ[?üÔ¾¹
Ó'?Ò+ÖÝò¹ñ?̚Ž…ia?ò‹ºc=¼ú@
^<™8u½?ÙcqT2U¿íR-ÿ틉¿³:è‰@Ü¿ÝÊë€ìúj¿é",<žìÀ¿Î{ÅHIúAGNbll1RXS J160709.7+592115?ïýp_¨Jü?'È͕¾j?4}TyÝ?'È͕¾j?ïöL9-?X
ã?SßòàÜõ÷?X
ã?ïÙ̀žBm?gÁEjýSÅ?s?™q‰?gÁEjýSÅ?ïø—iϸ¡?3$)è˜eÎ?M¢W͒È;?3$)è˜eÎ?ïý:@È?4uTÏLé?6-þ®ilŠ?4uTÏLé?ïÙK´¼?u,·ëš‰?sZ%èSZU?u,·ëš‰?ï¦uËQˆ?"šiâŽx?†bH:qå?"šiâŽx?ïñ²à°@?G²
Ä̱?\›ðA_0"?G²
Ä̱AGN4FGL J1607.0+1550¿Ýï"žKÁ0@E³ã*cÇÀ8•Ü¡u0À;͇®µŠ'@{/bÄw@"mH÷Q?¢:ƒ<=¦‡?¼i€0M6@80yþÊ@g~igw³?ïÈtþ¯è¿Þî|µ]D¿äYÝâìпäZÿ**¿¿çp²Osڿ鿞EÐÄ©AGNbll3FGL J1607.0+15514C +15.54?Ý¿ˆøGàû?ÓWtOLY?á ;ƒÜ'?ÓWtOLY?Ô¬gåÊþ?ÌëKüU?å©Ì
€ñ?ÌëKüU?èâ-:årû?°æí&¸?ÌwKj4?°æí&¸?Ò-5A*?²Í¨¿dIû?æøiuå_k?²Í¨¿dIû?ãîºíɔ?ͪZç­"ã?Ø"Š$lØ?ͪZç­"ã?·ÆÚün?ÂP`[›˜^?í=Ä[º?ÂP`[›˜^?ë/=pßø4?­#ÌD™?ÃC
<€0?­#ÌD™?›i®ê?ŽÑ¤Q1?ï'Côª?ŽÑ¤Q1MIXED4FGL J1608.0+4949¿éò"@äC-@G0dÜY2À;d»—cYÀ<ëëºÏ@Œ¨N"5ý@'<?ÓÞ>ɔ^?ڙ‡%"Ï8@8OLnmœ@ék'…?îü'"ø¿©˜ P`¿âôu
œ;¿é5ðè5 ¿ß²¢\¶º¿ïýÿ!]ÉAGNbcu87GB 160630.8+495728?ïûu l??E	>Ço;?B+€™½à²??E	>Ço;?ïñËï¿?`AË ­#)?\iýÃv/?`AË ­#)?Dϵ,?€O;tó¹u?‰ž.Öaˆø?€O;tó¹u?ïë<…ÜR?J©ÛNàë?dÃz<«Ý·?J©ÛNàë?ïúÖ±Ž>-?@ú`€Û?D¥9òu-?@ú`€Û?ïΝnP?yz⌊?x±vAg3Ú?yz⌊?ïbI3$Ň?N|tKª™?"¶Ù™¯?N|tKª™?ï²+e"]g?t
J·ÙRœ?ƒu&ºØBG?t
J·ÙRœAGN4FGL J1608.0-2038?Úñ(¼Œ¸¶@6'¬dwxÝÀ9㋘O¿À<hXÓ×@…€flÆ}@ž§b¯ø?¶‡a!œÌ™?vàé—çE}?Á>ìdl¼@õ+ÆWgÆ¿åù§4ƒ?¿âEB;å¿âsáxU|¿ÞuÇ,yÜ¿åOv_Ø­¬¿ÕqEiÃAGNbll3FGL J1607.9-2040NVSS J160756-203942?ïþ1n7@?!àk]íê?,îö€¹?!àk]íê?ïêö"š§?z—ÖËD?e	l]åE?z—ÖËD?ïôݲ£*è?a¸Ÿ2|?VDšö#Oì?a¸Ÿ2|?ïûÈ©¸±É?/-5m'?@ÝYH§?/-5m'?ïüÎ܋J?4˜©p?9‰ˆåyv?4˜©p?ùÌÁ?"ö¢A˜?ˆ^ok¡?"ö¢A˜?ïíÒ#m?q•¶)'?b-ܱm2?q•¶)'?ïò]ëºñ?Phñ:.?ZÅDˆ¿-‡?Phñ:.AGN4FGL J1608.3+4012?ÞÍþâ.ïé@GÊʁ˜ñÔÀ;‡³-¿UìÀ<î™
'¡/@'0ÉKó?û(¥U~Ž?àÒèÛ­e?ᚮÂu°Ü@Q¹eç»f@Yuƒ?ïئõ¢¯¿Ú´ÈÊÍ.¿â›W¿"Ç¿Ú"K©¢¿ïÿûÎBÓ¿ì—æpâÁ+AGNfsrqB2 1606+40?ïôx½«ò?i³®j¤u(?W"Ôæy?i³®j¤u(?ïæM[<?sY'QX°™?i²ÿwi ?sY'QX°™?îÍ¢m±<?""þš•¼?£%Ù'ôø?""þš•¼?ïš	Õۃ
?p>.Š6¡?‰}Š'@Õ?p>.Š6¡?ïÓ"_²‡?z'(n¤DŽ?vx6Wô?z'(n¤DŽ?ï¦%Ì\(?'K_÷»?†|v'š!õ?'K_÷»?î6{Ÿˆ›ð?žÜ|
Ù?¬˜FšYû?žÜ|
Ù?îç"®"4*?á°ÂQµ?¡Õ':i?á°ÂQµAGN4FGL J1608.7+1029¿àDÙl~"—@Dg7âÅ\–À9($}ÊXÀ;æÜ0@úñ£Eë@©æ~Nº?°¦3
9?Ä^DC{Õ¹@Ęވ¶ó@*
díj|¿Ë™à¦ÉWø¿ä«±^²<ÿ¿ç^Á÷†´»¿èÓØYÉ¿ë†Á½¥¿ðAGNfsrq3FGL J1608.6+10294C +10.45?ïÚŽWq+?qXU¶{¶´?rõ¸Ì¸F'?qXU¶{¶´?ïì+e/[?rT?Æ24¡?cԚ°÷­l?rT?Æ24¡?ïUi¨Ý{¾?kîðËö?•RÊéwò8?kîðËö?ïøœÊY2ª?7×Jo¿‡?MŒ×‰@­Ì?7×Jo¿‡?ïÀ͋ʵ,?vÛÑ&Ÿæ?™:+#Š?vÛÑ&Ÿæ?ï™Zc<ª?•ßë-M$¨?‰©g-eݸ?•ßë-M$¨?ï$Øԏ[J?"ÀU÷׈*?›dån–Ì?"ÀU÷׈*?ïß cµI?a5»Êƒ2Û?poÎbWÇÀ?a5»Êƒ2ÛAGN4FGL J1610.3-3958?ïÍqZ`HÀ@!îÐ,ӞÀ8û²êòÀ;hâ·Ý!@O=yÞo@rÓA[#?´&òH‡X?¸'­¼ç&•@| fèl@n'ÏùR?ïÿ1£æúu¿åaRàø}Ö¿çm͘¤§¿ç㺺{'q¿æ%ہp'õ¿ïýYÝl[AGNfsrq3FGL J1610.6-3956PMN J1610-3958?ïýšÜ 
"?'Î&LÖf?3) =Y5—?'Î&LÖf?ïÐNLœÄO?'Ó[‹YÎr?wØÙ½üpn?'Ó[‹YÎr?ïÖ(Õ÷?sYþ"ÙŠ?töëtyÄÓ?sYþ"ÙŠ?ïÛ×ú}_&?XÒëº@µª?râL¬§?XÒëº@µª?ïûpOY•¯?:êP;l?B>Á• p?:êP;l?î3¸GjÞ×?¸£ª3Uÿ?¬Ä{‹	à‰?¸£ª3Uÿ?ïŒ[´lêË?ˆ.à˜O¥V?Œé×ÝK?ˆ.à˜O¥V?ïñ+7!'?‰"ûÚi^?œaڟûæ?‰"ûÚi^AGN4FGL J1610.6+2414¿ïý4äcAn@F©A(¿<À:ŠŽ›8Ö
À<W[ìà³@ýI¤¹³@@ëGâàí?¹Áµ¢®Á¿¶[¬¤
eï?û=L¬€üë@5ƒo‹©¿áÌ=]º¿ç+{؃¿ë"9`÷ã¿Óe="[¿å£ÚЛŽf¿ÔÎ9´V´BAGNfsrqB2 1608+24?îÃÝ.¼"}?Èy\ÂùN?£Â-õ¦.?Èy\ÂùN?ïï¤& ·A?gåâ>™XÚ?`[ÚÃá?gåâ>™XÚ?ï×ÆS>Ÿ?yr¨$¼?tÖ`""?yr¨$¼?ïó—Ók?B;±zbÊ+?XÑԞ}Y?B;±zbÊ+?ïßÇæ³þ ?€)°ã˜,e?pˆtR?€)°ã˜,e?ï±Ó¿I?ŠŠÝxsä?ƒ¸‹	þmn?ŠŠÝxsä?ï_3È&]?">«Ôˆ?"‡3k?">«Ôˆ?ïg·Cù?†…
ÜËõ?"	Q?†…
ÜËõAGN4FGL J1610.7-6648?î}Oó¢À&EÌBcQßÀ80äÅçÖ>À;]C¢ìÿr@m‰'8Ìû?ùÑb§•?£rRØ¿õ?¼fý4ÑC@¯Â¼¨'[@Ëïž]ù…?ïýÆ¿Âx5¿Ë‰ g¿¿ÓPÛ$Sql¿ÒjCÒ ¿ÚÒTჾ¿Þ(ƒÕ,ÃAGNbll3FGL J1610.8-6649PMN J1610-6649?ïç'Ü4k9?‡Z琢?hØ#¦xÿ3?‡Z琢?ïƒ>iœÚ?—iXŽU{"?0{ÚY?—iXŽU{"?îôÖcùÎ?™¼zÆÏð‰? ²™Ðä?™¼zÆÏð‰?ï¸þZÀœ?n›#¥0?Àin°ñ%?n›#¥0?ïÉÂü5èg?a2?g¢?{ã«ô®?a2?g¢?í}^v>0ù?¾ôCÍùâH?´Nx5?¾ôCÍùâH?ïŠf†"&?'ù`¹A?{&W{¾?'ù`¹A?ÏÈ?"]A«oO±?¥Ç#Ç1V?"]A«oO±AGN4FGL J1612.2+2828¿ï
z@FóI{t¥À;j€G¸ü5À<É~#òM@ˆ0,–?þ6§¬Óª?Ó6^á·Àv?Æô$j Ü?òÍ…/?ÿz·^P˜I?çÿMR8¿äwý''i¿ÑE†\{&¿ãþœÞGžz¿Ö`ŒÝž5¿ïÿ®©ÌAGNbcuTXS 1610+285?ïð®4Êü­?[†E"¾ü?^£–'†ë?[†E"¾ü?ïëSjW¯?h+‰NPxœ?d¬•ç‰ÄÁ?h+‰NPxœ?ï·öTî?}¥mtµÒ?':B‡Á*Y?}¥mtµÒ?ïÍÎk¢?[¿‰‡£õ?yó·2^ß?[¿‰‡£õ?ïäb'Uät?h®8†0¥?knšýCÐ?h®8†0¥?Ïmf?˜›Du˜?ˆ]~þf6'?˜›Du˜?ïErYL?"	טxtj?—Q¾vŽJÞ?"	טxtj?ï)D¹å¶Ë?‰yèãԇI?š×hƸœ?‰yèãԇIAGN4FGL J1612.4-3100?î³DÁX­õ@-P¯>FŒ¬À9a³õerKÀ;ÐôƒÊû;@µÉ¢ö»?ÿiðÿ±üg?²ÿÂÊí?Ár^—:@¤[^Ëgr@7ºC³3?ï÷T?NÛ¿Û%î;²]¶¿ßö"ºÝa¿ÛüÚ\¿çÄqê('f¿å	BsíãAGNbll3FGL J1612.4-3100NVSS J161219-305937?ïø8µBx?UcCÑ þ'?O* €Ýû?UcCÑ þ'?ïÒe!0Á?…JÝÐ\?vÍomß
?…JÝÐ\?ïÑZÿ¼?x$©.?wR€<
¿â?x$©.?ïøIÅ=Y?5ÔB¤]@?OžØA<?5ÔB¤]@?ïø€ƒ?NOS»¼@õ?Mÿ²Y"WÊ?NOS»¼@õ?îœ,.dÊã?²CÞò¬>ê?¦==8È?²CÞò¬>ê?ïŸÜ²Ú¡?Š³T¾Ž¿£?ˆÓPYº?Š³T¾Ž¿£?ïç͘"y?T¯Q+º?hø2qnë?T¯Q+ºAGN4FGL J1612.4-0554?ï¶UôB @?C«CIIÀ:pHD<oóÀ;÷žXE;s@y5ËéÍä@­"'±È?Æ=vƒ? ŒÂ_zRÆ?Õ\cÞл@5H
æš?ïþ_ìÏ¡"¿Ö†—^Uö­¿í´4 ½¿Ó#>ÿP3¿á‡£,ÀRk¿ïÿý{ÁA~AGNbllNVSS J161228-055752?ìújܺ"?ÑN̲±Ôµ?¸,©.ï?ÑN̲±Ôµ?ïë¯'9C²?ogçîWá9?dPض>-Ì?ogçîWá9?ï'©;<?–axg†&>?›
ؓWõ°?–axg†&>?ïôjø"Çj??·©5ˆ÷·?W*-§{'??·©5ˆ÷·?ïÜCÊ/?x;^‹º?qó÷fYøX?x;^‹º?ïcžJƒ[ë?£­ÜWë`?"Œ6¬$æ³?£­ÜWë`?î™%Q.'? Ûi©¯?¦mªï«"±? Ûi©¯?ï½Ù@ë?q¨<Ó"¯á?€¸‰¬63T?q¨<Ó"¯áAGN4FGL J1613.3-1907¿ïÆ	t ¢@6®g¥*ÇTÀ:°Ä±uXrÀ<‰X=@ fÔÜeÇ@™×ºf˜»?Éé'¶Ó;Q?¹hìÓ}k?Æ£ÌùBv@ºØØãÁ?ÒO.¦Üx;¿æ38q`•l¿à㠀þî¿Ùµ
¸A%¿ìÀÊ*Ü?Ó㻹ÿìAGNbcu2MASS J16132720-1908364?ï÷-=ÐÆ?L`}°~¬¬?Q¥"=w¾Ø?L`}°~¬¬?ïîb:Kš!?d•‡j²ÆO?aÅ±¦.ì?d•‡j²ÆO?­#ua?‰¬·*9"•?ŽTÁq{£?‰¬·*9"•?ïùlˆ>}i?5î/ðÛQ?JMß¹BÆ÷?5î/ðÛQ?ïø÷Úu5?R@¤sÞè7?Oø Kóž?R@¤sÞè7?	쬫?—¡btE×?Ó}ˆDqD?—¡btE×?ïŠPç}?k½pìÚ½?kÛ»ë°?k½pìÚ½?ïáçÝZŸÅ?^Ù¶*p?n"ǼRè?^Ù¶*pAGN4FGL J1613.5-4225?È(̊ª
@H)ŒÁDÀ:P#tƒÀ;'I:µL@czðáÿå@€c?jy?Ñͤãú'?·aÓȌv?ìÿMB}þÞ@ˆád3†?¿ïôµ´'S,?ïÿÚáb†¿ìõ¦n"¿Ù±ÙŒÂÇ¿æú"ˆ¸¡¿ÚŸ)ÜvAGNbcu3FGL J1613.4-4222PMN J1613-4225?ïô¬V×õ?pMN²S›|?WÖ¦ï[U±?pMN²S›|?ï·}è®?'ã?ĪÙ!?' †SÞ7?'ã?ĪÙ!?ï O'c?•Šª,R³?›ö·;Û?•Šª,R³?ïíö-"¦?J>ïcë†?b	ïÓ?J>ïcë†?ïxà")î?˜–÷sëê?ãízÂ=þ?˜–÷sëê?햊qA?¼ŒØ»ÿ†?³K¬v¢?¼ŒØ»ÿ†?줄à‹+Ô?­S€DXÖx?ºÛØû¦¡a?­S€DXÖx?ï:-Ôµµ•?Œ‰°|æÙ´?˜ºEqàSN?Œ‰°|æÙ´AGN4FGL J1613.6+3411?ÃNJ°þ:-@G0Nø‹—xÀ9*E†òÍèÀ<DÊPñŠ@£KëW@Y䒼/Ç?¦»®—WŸú?Ÿ–k;ã0?óFÌ¢Ûa»@Ñ´ì–¿Îú"€'ÇE¿áýÔ þþ"¿æbE'Ë¿ç~b †ˆE¿à'Tჾ¿ïÿ‡¿ÒhmAGNfsrq3FGL J1613.8+3410OS 319?ïý2Í žu?+€ÜÕYN
?6i—ØÑC?+€ÜÕYN
?ïöN/þ?SÛ<@ó?Rác¹äó?SÛ<@ó?ïèË+ÉÈ?jòZÁ½³?g4Ôw€ßø?jòZÁ½³?ïú£@¶Ö?8%5x‡—?Es¦®?8%5x‡—?ïû¥á.6R?=¯LØäN?Ah{m›®?=¯LØäN?ïÚë"ü\?wšÃh\¤3?rý
@Aß?wšÃh\¤3?ïՔ…nÐ~?xÃÝщ{?u5½R攻?xÃÝщ{?ïô^#vҚ?Mã+Ç Àá?WC¹"ŒÊ?Mã+Ç ÀáAGN4FGL J1614.8-0850¿ám×*b˜ë@=É>¢ÒþÀ;7x"væÀ<_"\h¶£@"җ֜Y?ý+G&/>²?ÆeXŸSl念)f€½¨?𗐪ݎ¼@~I‰¶Í‡¿æœ"¤?¿ìGðI´¿×ôƻ栈¿éùqÁ
{꿳Ce/"§ð?×â•@ÄkTAGNbcu1RXS J161443.4-085130?ïýÏÁ?D-ßH
º?7q‡y'?D-ßH
º?ïçh‡'üô?suçØïB?h—xØÎ?suçØïB?ïŘ	Ê?¼wLy¶?}3ÿê?¼wLy¶?ïý^µŒ'?+°†‡ã?5
VÎ~<¡?+°†‡ã?ïüò™\T?G‰¸Á‡Æ?8k3œJ™«?G‰¸Á‡Æ?ïEˆãhð"?¦ŽµcD`?—N㍺…{?¦ŽµcD`?ïÎÄÎs‰?€Ü­)>HØ?x˜Ðȏ8?€Ü­)>HØ?ïéœÖ‡X?eÌ;C@Ô?fc)6¯ep?eÌ;C@ÔAGN4FGL J1615.6+2130?ïò
Ãl?³@E¸óË>WTÀ9ù9&BÀ<?k@Àºp@˜÷-žsÉ@ëÏkn
?¸aöKKX?¡¶m嶩?áMp€ñ'@\"òB¨¿Ã"ïCDMb¿è8ÁצE¿ëhÎUcä¿ÛÅ0@'/¿êÃJ¢»K¿ïáñ¿Ë]AGNbcuSDSS J161531.09+213011.0?ïû:ïü8?<H\hQÁ?CAâ?<H\hQÁ?ïô²­Dyà?i~ïٞÉ?Vš¥ò¾/?i~ïٞÉ?ï̲vÆl?ydÀão?y¦Ä…lš??ydÀão?ïø˜Æ=š?9U‹™xh?Mœç¼C;	?9U‹™xh?ïïƤ"Ÿ_?aÞõ™¬?`9[-‡©€?aÞõ™¬?ïÑ#ðÂm?€
-ú÷—?wuíì!éÄ?€
-ú÷—?ï¹'þÄ
-?ƒÑ"—…!ý?¶[³B­?ƒÑ"—…!ý?ïàèˆÈ™•?]®ãÊ>£ç?ow%ˆs)?]®ãÊ>£çAGN4FGL J1615.6+4712?¤g~
}ë3@FÎãK"SÀ:C{À<‡)éÞU‹@å5oùb,@GÇ$_¾?µî@dô÷8?¨f*ßÛ%?òŠFu/W@Ÿ´Ú'³ ?ëw¨¾$¾P¿Ñ´]¸½¿åMI"žˆ¿ßéþ Õ®¿ã&óõ/Âe¿æE£þwiÄAGNfsrq3FGL J1615.8+4712B3 1614+473?ïýÛøä­¿?!d)9 f?1 8P.{?!d)9 f?ïóm>`¨?[€ñÉÝ·\?YÕ%ËÑW?[€ñÉÝ·\?ï÷:(gI³?U63º?Q‹¯œ j/?U63º?ïá²eÿt?TW‡Àoœ?nïM½¼{S?TW‡Àoœ?ïúèÒ£?>6ñ3£Œ?GÐ[¤9HÐ?>6ñ3£Œ?ïÓ×TTý?wTÿ'ë,c?vU;ñŒ?wTÿ'ë,c?ïõÁ¯|Í?b%ìÙö–¡?T|¡¶ó?b%ìÙö–¡?ï ´&Hû-?q‹ö(èB?‡Òö{¤¼?q‹ö(èBAGN4FGL J1616.6+4630¿êp¯Nÿ¦@Fœ¢ß"yÀ:ØÐi9~À<-\6@øÓËCµ·@±PÚãæÅ?ÅM-šÂäl?»þÇƨ›j?ñoxäl-@CP¿Ê^ªïj\¿åƒ]b[¿Ä¿éR,†pÈ¿ì2àÈ,T¿ïùÕyC¸¼?ïîê>!βAGNfsrq3FGL J1616.4+4631MG4 J161600+4632?ïþ"‡—õ'?#Éy–†´?&džåÎ¥ß?#Éy–†´?ïõeÞ3Û?X 3ï=(?U4Cz
m=?X 3ï=(?ïå8ސ;?p°¨B¡Ï?jÇ!uDG|?p°¨B¡Ï?ïùP^šÈ¡?7¢Ö©5?J¾†D<½
?7¢Ö©5?ïý®y®?7†+Xs;m?7)–­?7†+Xs;m?ïÑÁí[ô¯?zÙ¡¸G<Ô?w	QU¼¯?zÙ¡¸G<Ô?ïÝV‰¾c?w‡ÿ†:¹?qTø£î¹?w‡ÿ†:¹?ïÉõB€?lMŒoz?{_íý@?lMŒozAGN4FGL J1616.7+3327¿çS
g+Ö@FÖÄ`퀡À;ô/eƒÀ<¯'ÎÉý@g(<	E¤@:#|ÜÊq?ÒÛ<'¦?̍À‡ïø÷?øì#>Éik@vþöj«?ºÂÊ?~Æ¿é"i†¬W¿·™y¹)'¿á`àpÀ¿æëg@ò¹¿ïøUFƒrAGNbllNVSS J161633+333043?ïîTr"="?c¢ËÑ?a«Šá%º?c¢ËÑ?ïîÜ-'à?cwa°|
²?aü#ÿÇ÷?cwa°|
²?ïÏâ*ðo?tBÆoÙ¶N?x÷íGx³?tBÆoÙ¶N?ïÊ?³ìx†?Zz,Jò{¸?zà&',ß?Zz,Jò{¸?ïé6##y?efÕ?ê†?fÉý§BŸ?efÕ?ê†?ïÅrvÅf?€`ö—:¶?}FÄù,pÞ?€`ö—:¶?ï_Wë=??¹S߀L¤?"
õàŠ ?¹S߀L¤?ï@L~]Óñ?–j²rÐÏ?—öp7µæ?–j²rÐÏAGN4FGL J1616.7+4107¿åగ7½@Fúù3]$žÀ;îgQGñÀ<ÝÌúïõÇ@p@'Òë@Rºà;>š?ÇFBšvØ?ÆðÀU?üª«õ¼°@I+®Ús~¿æÿb`ÈAο³ï(nß¿æ''àðp@¿ãk¥Õçþ¿êžJ''¿ïÿý¡UûŠAGNbll3FGL J1616.8+4111B3 1615+412?ïæ6'%Ö ?k§|d4G?iÉÙC'Ú?k§|d4G?ïßY»Ìä?pÁÈJ#À?pS"/‹y?pÁÈJ#À?ï¾ÎÉôw®?vXCž?€LMx;JŽ?vXCž?ï›ø9j¸c?iºì"r?‰ñ"#ÛI?iºì"r?îÈ
z¼ßš?£!œüöA?£(SVd?£!œüöA?ïz[Êh?™#ùºe?´ßÓÄ÷?™#ùºe?ÃSëÿ?šÿk -ž©?¦ÔCÉ	r?šÿk -ž©?íš1#Zð^?œÑÀSLH?³.værW?œÑÀSLHAGN4FGL J1617.2-2535?د€CºÈq@1£Ï_ND1À:a-ñªÓÀ;Ñ}‹Q@ïՃ)Á@™ð^¢LÇ?Ð;¹eç»?×ÑË9NÖ'@¢þ'Q~x@ü¹"`ʛ?î´º𠏿ÑW³°œž¿áÌþ ÚU¡¿éÒI
{¿ël‡þ¼'¿ïÿþÐñAGNbcu3FGL J1617.3-2519PMN J1617-2537?îä6çP?¥–_ʸB?¡¼ŸßØ
?¥–_ʸB?í'¹Wz?´É~š­?·.Â4Ö<?´É~š­?퐆Að?£ßï™ti?·|;ãý?£ßï™ti?î5‰Z˜c?Šþ_"Œ?¬§jSæ?Šþ_"Œ?ê@ÈÐý^?Æ|Ø^·?ÆüÜ¿´
‰?Æ|Ø^·?ߋX_ès?Ñ
áÆK?à:pSÐÇ?Ñ
áÆK?â‡m>"2?¹ú{ÂÕ8g?ÛÎñ%'ל?¹ú{ÂÕ8g?âÌÊ.Èü?³µA'x¸?Ûúfk¢n?³µA'x¸MIXED4FGL J1617.3-1513?ääÈԒ
@8†Šar
À;Dèg]À<¤Ú/­m@ t‡t~8?ûÞþ'¸«®?ÒÃöúȳŽ?ã$ì^¥«@
ü«>݋a@b§¿÷ý?îA$øÝÌÏ¿åwÿ ´•ô¿Ã"žWïU8¿ÑM²¥Ú¼¿ä·Z¿êU¿ïÿl\I¬òAGNbcuNVSS J161713-151058?¶S}?)°5cûW?‡WyNû"©?)°5cûW?꾌JÚ!?ùÞþ)Ö?ÄõÎԗz?ùÞþ)Ö?î‡6©â?›½yIwU?§ü'Ü<â?›½yIwU?í%QL'™?•?ït»•w?¶Õu#†?•?ït»•w?ï¶C‰u<Ì?Eú`-è?'o¯e	?Eú`-è?ÞIŒJô?Òd^BšH/?àÛ9Úõ¸?Òd^BšH/?êJ‰e'Kº?³‡e÷Úb?ÆÕÚiºÑ?³‡e÷Úb?ãîÊ£|Ç?¹®Â­†'Þ?ÙÜ"j¹q?¹®Â­†'ÞMIXED4FGL J1617.3-5849?￱'ÍÀ¶R7yÀ9>Ì?ß À;"ˆ9@"שÇÁ@ŸÜ>Y×ã?µM16-äj?Î;y}ÅR°@Èa-A'@NÔ¤\–?ïÿ¼®q—ó¿ãJ;ÝüŸù¿æ^:é
5¿æ2qôÆ¿í"t¡'Œ_¿ïýÍ ²<©AGNfsrq3FGL J1617.4-5846MRC 1613-586?ïƒP±73ã?ŒRÞ\1Ó9?+Ó§ä3f?ŒRÞ\1Ó9?ïÏ´D"ƒ!?Š`Su¿?x%ÝÌ,ˆ?Š`Su¿?îC†]ZVÁ?žc³wd†?«Çš,îHé?žc³wd†?ïÜí"ÃÎ?Z]'+e!V?q‰6…Ý)?Z]'+e!V?ï)£—@Æ;?"wµY˜Á?šËŸ˜?"wµY˜Á?{"Û?³øQg<)p?¦">ÙþI?³øQg<)p?顲Œ?°•a£'Á?É{™7Ï¦?°•a£'Á?îãqhðPØ?œš2¤J«?¡Èél¯o‰?œš2¤J«AGN4FGL J1617.9-7718?ç²î–2˜À2ÞM;òõVÀ8tvÔr³|À;²/,=u¬@‹Rùw$Ð@ƒ'?	*K?¡.—3M_?¼¸ÈúÃ@À‡Þ†2µ@©Ö¨˜»¿ÖýCãÅÝ¿ä…dXo,ß¿è™Ì$0`ñ¿èH*;<ìð¿èS½í5øà¿ïþRúÉAGNfsrq3FGL J1617.7-7717PKS 1610-77?ïüi+"ÿ›?3Oß(I¹j?<¶¥¯ÀFÆ?3Oß(I¹j?ïîÌ¿$²?}Ç«æÕ?aè3\X-"?}Ç«æÕ?ï¼?Ÿ¹T†?'[üMé´?€ð	ve?'[üMé´?ïý¶‹ås? ý¿»¡+?2K¡°ÈsÏ? ý¿»¡+?ïþ‰<Õ?+ᣀxj8?/÷oEî=q?+ᣀxj8?ï͐§,ª-?§ƒÑ?y7¬qéùm?§ƒÑ?ïnjó35?r}<>?|9ôe%D?r}<>?ïóï'à÷?Ný¼Èzøq?X ۋ
C~?Ný¼ÈzøqAGN4FGL J1618.0+5139¿¿ú3ÉlVQ@F8AVâeÀ:Žf$ø
À<ž0´Ó±Ã@Ua÷ÁÃ@†6Œs?˦>m£ò?Ìd6÷—&?ýñ¹KÈË@µ"Üž¿áÊ~ŸBP¿âÐ{÷È¿ç=xÁ‡Ê9¿í8Æ_ö4пåF/ßÁœ¿ïöØmAGNfsrq3FGL J1617.8+5137TXS 1616+517?ïý½w8ø?/[çe7?2FR?/[çe7?ïôX=È|J?Z»ÖJE+?WO"«ú?Z»ÖJE+?ïКžk)?q»ÔЦôë?wÿ²¬ªãW?q»ÔЦôë?ïþ94ËT?ڗœd§?,lÀÒ&€®?ڗœd§?ïÿ-ß%-Ñ?)>½v*
?D0I¦5?)>½v*
?ïÚÿ%B7f?rô"c‰â¡?r€mWU)8?rô"c‰â¡?ïXÔn›'í?ÎÄ¥Š3b?"år) q?ÎÄ¥Š3b?ïùY¾ç ?<¾³¡°þá?J›'»¦€?<¾³¡°þáAGN4FGL J1618.8+0620?á¡ãü$@BQAAé¯\À;5¢é¤sèÀ<šè¯bk@*s6›f?ý™yƒyœ¤?×3Úé%?Ô¹‹|uqq?ûŠ'5Îï@ëyÙ	ññ?ï¶`^åh¥¿ï)BUæ?í1Ý'ãƒ¿àtž7ŽÇ¿è÷ôÎs•ú¿â.ó2'#"AGNbllRX J1618.4+0623?ïè-Ö|?c›šENG?gÒ*?`?c›šENG?ïã{yaÚ?r{݊¯¦?l"†Ê €l?r{݊¯¦?ïs?þÐñ?‡Üi°šR?'˜CEÓ?‡Üi°šR?ï}¢öºƒ?xZ¿œ2ø?K¡>(¯¢?xZ¿œ2ø?ïÃÞ¬s;?"õV3u?~©¿ƒB}?"õV3u?ïe?{Q@K? AÔ'2i¢?"X™G'¥? AÔ'2i¢?îËv:¸?˜&Ü	¼~?£HŸ?Æ €?˜&Ü	¼~?îóu"!Ée?'9-
^¯Œ? È§ÁS±?'9-
^¯ŒAGN4FGL J1619.0+7536¿ä{¹šý@A¨ôàM/À:˜NHboaÀ<Ç>óZÖ@7*Èü@:dÜY?ÁØÍ÷o7Æ?ÛŽd9îí?ÝGåœÒ^1@D qúï¿Ò3 ~O¼+¿æÌè`§	Å¿âߟb[j¿Úa(	3…¿ÕÙôÌ.A¿ïÿÿ&¦³AGNbcu3FGL J1619.1+75386C B162034.5+754454?ï÷œs™!?S˜6%T›?PÇ­ÎJ?S˜6%T›?ïöa"h¥?VLëÁÁ?S=ÐUýgf?VLëÁÁ?ïî¢Ø\¢î?e˜ƇQƒ?a]'Ë8‰?e˜ƇQƒ?ïòþEt
?@©A8«‰5?ZuîS61?@©A8«‰5?ïô+HX3s?Qãù­Ô?W©o+Ý*Ÿ?Qãù­Ô?ïÛù‰Q?qŠ7ýv{›?r;8G²?qŠ7ýv{›?ïé'|G¤?sáh£Öª?f5CV]"?sáh£Öª?ïӄ«ª?aâÆ4Žô?v=ªPè"-?aâÆ4ŽôAGN4FGL J1619.0-8346?í¼Ö ]æÀ71qâ›k+À:õ6¥®zÒÀ<.Ï d$@¸½Mþ»‡@ú?¤Z½¼?ÉõMõVXÒ?¶s€wµ?éؽf'|F@,9í±?ã£Æ
•ê¸¿Ú•yyh¢¿à»²]µ½½¿èA•\¿æ;Þ§j¾¿Ì9\-AGNbllPKS 1608-83?ïüþŒs§~?1…"³NN¼?8œ¿÷Æ?1…"³NN¼?ïòl4X?Y\6cË ¸?['—ØQå?Y\6cË ¸?ïßÒ¯Kè?pøzsVö?p¨IFQ?pøzsVö?ïïµ¥=ç—?Aº'¤ï£?`JZðÓ—?Aº'¤ï£?ï÷[G4®?G¤ÏÌýÍ?QIqO+îè?G¤ÏÌýÍ?ïËwϼ¸¥?~áÃÚUæ'?zD	²?~áÃÚUæ'?ïÍÍ|þŒ?€hrd‰]?y})sv,?€hrd‰]?ïœp~½[?rÊؼ©B÷?ˆãù™qq+?rÊؼ©B÷AGN4FGL J1619.6+5536¿í'PÆÛµã@E¡Þ?»×²À:†—¨'ÑÖÀ<³¯' Wú@5ÈRi¯F@õÀ[¥BD?Á7;ÀöTÛ?À¹‹§h6?ûIKRä©b?ûÜP§¿¶abEšh÷¿ä‰»j¤¹ˆ¿åê™ÑͽŽ¿æ]¤öÄíÛ¿éÜ5 uÖÇ¿ïý?ÔVYAGNbll87GB 161814.7+554307?ïëK¿nP?b[Ã8*˜?d´AQ_«?b[Ã8*˜?ïS·o˜iC?68khm?•‰Ëm«?68khm?ï¹µ"þ­£?zÞÒͬõ?'šïÖwQ?zÞÒͬõ?îAÙj‹?ô¹³'þ ?«ânº;ÞO?ô¹³'þ ?î-¶g?¢.óÌT§®?¨
/¢áÀ?¢.óÌT§®?ëE›¸'½à?Áìãð¢6n?Âé'õ€?Áìãð¢6n?îÄ.IÖk?™
Ý_´I?£½z†²K?™
Ý_´I?åP"9v?³ràOÄ?Õ^÷ãà?³ràOÄAGN4FGL J1621.7-1103¿ïmJg'E@:RÖËSP	À9ƓX6ø»À;ò­×>?×@‰s,Û*@ÐÈb?Âz	2®?ÊÕÊw]¼@7E«I@r 
´®?ïƒ=lr"¿Õh'{Mz¿äœ»sG ¿çÝ]Ó6¿ïóüQօ¿ï¢æÿþÓZAGNbcuPMN J1621-1101?e¨?•'Á ¦?ˆºÞÞ?•'Á ¦?ïÖ5ð쀋?'Y¤>ûÏ?tåx'®‹?'Y¤>ûÏ?¦±|‡?˜++»?§6E"P–?˜++»?ïÖpJH,?^óèš0¶ã?tÇÚÛ~ ?^óèš0¶ã?ï'l	ϝÉ?Š‹ûÜÙ?‹¤ý–gaÃ?Š‹ûÜÙ?îÊèb»?²¯p#Ÿ."?£_'yÔF-?²¯p#Ÿ."?ë)ђ¯D§?¬‰ŠWy'?ÃX¹µBíe?¬‰ŠWy'?ï~Vvs¶?€4Ò·sÒf?511©@?€4Ò·sÒfAGN4FGL J1623.4+0858¿Á½Ê>
h@BpJb#á‡À;a)ÄÀ<Œ«Ü'<®@ \<
<ç@V/Äé©|?È0§$G¿Qq±‰@4CºêÍ?ïü–ô£«k¿Ô톀¸!D¿ç|^?¦^#¿â?ü¥¬¨?±yÃeoñU¿ïÿÿ)@k*AGNbcuSDSS J162330.56+085724.5?ïû4â	õÍ?PâQKP¦+?C,xl-á?PâQKP¦+?ïðšûL½?o¾sü¥¥?^Ê	—wK?o¾sü¥¥?ïϹ_°"?}ݒ>qÚØ?x#pQ‡–<?}ݒ>qÚØ?ïüåß í~?$ŸÛòÚ-?8Ñ;F®Œ?$ŸÛòÚ-?ï÷¿e?Z%õ'S8?Qþ'!»æ?Z%õ'S8?ï´ÐŽ§?'ÃUw"BÂ?'Ëÿ8­
-?'ÃUw"BÂ?ï°k-S'ù?‰œ$ç«?ƒå4¢GÚ?‰œ$ç«?ïóìëPF?RtӇ–'Å?YÊ&‰""U?RtӇ–'ÅAGN4FGL J1623.6+5743?ï€ÉÙät@EÅXdE$À;÷GʚÀ<ÝxC½@b*"y@ca	/T?ÃWSùÒ>|?"ãpäTäð?Ñóêî?ò*}'Þ?ïèÙ¨}b+¿ãC''%ο؉ }8é¿ãã'àp¿ë|'Biñ?ÇÈ?Il¶AGNfsrqTXS 1623+578?ïâ"9y?iOÇ"ûž?mlëõÖÍ?iOÇ"ûž?ïÈ,"	7?ƒ§9*É S?{éþ,\|?ƒ§9*É S?ï"Ł¡L¹?'ÕHऽ?›§O͎6ç?'ÕHऽ?îÑYNzâI?ˆ]Ã?¢êkš
l?ˆ]Ã?ﮒè®m?'Ò½Åzuu?"[EÛ]\?'Ò½Åzuu?î"ü1ê?¬…m¶¾wÝ?¦À>¤>c?¬…m¶¾wÝ?ïMÄ®g©T?'	æ7öÊ?–Gj82?{?'	æ7öÊ?ê´îÎn&?®LRGEp?ÇÝ,DÆGf?®LRGEpAGN4FGL J1624.6+5651?ɹ1Fkk«@E!©T!ÀDÀ:΢Ç?ÅÀ<Åð®{©@Qœ«qÞ?@	A=?½¼ËLïò¿FÚ«´XŸš@cý/ìð¿ï†'Ìͤ?ïŸà¥Ç¥F¿è6¯¿uÌ5¿ßQƒòÖL¿à 4óý">¿â[7(‹9…AGNbll3FGL J1625.0+5651SBS 1623+569?ïý[ëŽ.?4,Ñó¸?5 £¥¦ô¯?4,Ñó¸?ïõ@{g¡Ç?XæmÆ£±)?U	
@ÑÑ?XæmÆ£±)?ïðÓ[?g^š>)_?_YRò?g^š>)_?ïò=†b?C¹›ª»;È?["òЏøx?C¹›ª»;È?ïø+…¦?KÌ.")§?M‹R<kP›?KÌ.")§?ïÕÃù¿t?vÐ`½F}V?u.`'?vÐ`½F}V?ïð‹¡ðfk?iH\#'©?^è»õ÷Ùå?iH\#'©?ïʊhVß?lÁ9
­–ó?zºËÆ"Õ?lÁ9
­–óAGN4FGL J1624.9-4210?y»œ"@1ßv½À9°\'¹À;2{"¶
n@é¢[	;@,üœ?Џ½ei?äý®l@Zw¿á?þÌL&t3?ïê4†ðIª¿Þ{?[µˆc¿èß6üìOI¿ìxToÃÝ:¿ïÿþó…õ?è–ý]
wAGNbcuAT20G J162458-420657?âæ\Ô0?Î2Ã×ZÅH?Ú3FWÁ÷ ?Î2Ã×ZÅH?ÐàÖ¯yª¼?ÉÝæ‹ËáÑ?珔¨C*¢?ÉÝæ‹ËáÑ?çÇ·™p?¯—×t1y?ÐqûÞÍ ?¯—×t1y?àSóØ)wH?¶blâ?ßXO­q?¶blâ?ʟ^}éÿ?ÇV	t?éX(yà…€?ÇV	t?'ÇO|Š­?œ2£{Ä?ïqDž»j?œ2£{Ä?Ñ ïX=?µÐ‡A}Mß?ç/ýSá?µÐ‡A}Mß?"Ðjÿë?‡•%ø["?ïa|§ùâ7?‡•%ø["MIXED4FGL J1625.2-3600?»"('Cµ@"|ڐî¢À9ô
 yóÀ;"Œ"ÎX¾@4ìƽ>@Ÿ¢È…?ÉQÄð_y?˛?áíEh@¤åýö;?ürµ"¡ã?ïþ{eÑëð¿Ú1/"‡•¿é³iï‡â¸¿çØ-Þµ'ƒ¿â¤C@Çp¿ïþ
ýŠúAGNbcuNVSS J162522-355452?ïŸ}'ÙºO?‹ú™8Ë£'?ˆ ›B˜e?‹ú™8Ë£'?ìÁòE¸O?»1—£[uƒ?¹ðoåÒ=‹?»1—£[uƒ?î¯&Ú=o?•°w†¶?¥
'Zx+?•°w†¶?î¹9.õ¶Ñ?…Úœ»"rb?¤lm8Gî?…Úœ»"rb?ìïi9!M?» æCZ6œ?¸"¶5®#?» æCZ6œ?ԊékY?ЊÎÙ?庋|J~S?ЊÎÙ?æÍ•ö]?·Q"mö÷š?ÒeöÔÞF?·Q"mö÷š?â­óƒDîr?¼{¦êe"?Ú¤ùv#?¼{¦êe"MIXED4FGL J1625.7-2527?îÄ*©÷µ¯@0PÙÆ°SÀ7ÇϯÖÀ:ñq¤ˆ
%@JIOTQ@_3¡íûñ? :)­?Áªàú®‡@ n
ˆ~¿#@ —Œùù¿Ê"¸ç' ×¿áXß_vˆ¿äy`¿'F¿å(Ø0®µ¿éÜ°|¿é¹ÅÞñèeAGNfsrq3FGL J1625.7-2527PKS 1622-253?î|ù-†?ÉhPÇÿÄ­?¦(0hÜ?ÉhPÇÿÄ­?ï¾d²1@?‹­½N:ܱ?€fÓz2û?‹­½N:ܱ?î¿
ýM?šH['jz‰?¤/½šÆ9?šH['jz‰?ïü瓑[¡?1Gcj'â†?8ÃcT&µ"?1Gcj'â†?ïb›1¸ùu?'ӏ?"¬™Ã¹ge?'ӏ?í÷ÀJªÀ€?¼xLdT	å?°Aý«óÖ?¼xLdT	å?íL´ˆ!:ý?¤‹$
Ó?µš[Áé–?¤‹$
Ó?ïê†7"ë?]bÛË?ø?eyä‹òõP?]bÛË?øAGN4FGL J1625.7+4134¿ï¬ò'ØZ@F ±Ù+€À9Ê"
qÀ<qºnü7@‹#IWƒ@l¼Á¼ÎR?¶¨åf÷…Þ?ÄÍï»õå@êiæM§S@bÜʵ›¿ß¬;W¿ãÜâąֿæQ%AX¿çˤ® '¿ïÿ°7ßj¿Ð¸âÓõ5AGNfsrq3FGL J1625.9+41254C +41.32?ïõ¶bÓü?S•sì¢/^?T":õˆa?S•sì¢/^?ïðØQ),8?`1|tþ®>?^O])p?`1|tþ®>?ïÐé>Èg¸?sJÛ8"°?w‹`‰>?ô?sJÛ8"°?ï䮏ÁT?U*5ümÑ£?kQøu¾[?U*5ümÑ£?ïæ]Ó""î?jŸÞrµ¬?i¢,¬²?jŸÞrµ¬?ïǑ_Ê|!?~Þ³á
ÊÉ?|7P-ÿ¿?~Þ³á
ÊÉ?ï£|íe?•z"Å!?œ‹Z!`?•z"Å!?ïsWÌy?€‡.'¤?'•Isj?€‡.'¤AGN4FGL J1626.0-2950¿ïÖ=LDYÕ@*§ïZ–N‹À7ö¿Ñ;ÇVÀ;O«›úœê@L;kæÙ@§"ÁÄO? æ……x3?Á<'§º™™@Øņ‡n@EŒê߇e¿È«]üµr¾¿ãS–JYÀf¿ç¥mB"º?¿èÀ;Yrb¿éüc'í"Ó¿áV[áþ`AGNFSRQ3FGL J1626.0-2951PKS B1622-297?ïùÔÂ1	Û?KoEoå?H¬ö2P`¯?KoEoå?ï¾.xR:ú?Xû"—nu?€taõÀl?Xû"—nu?ïZ\²½­?'õ;æ<?"´pÏ´Z?'õ;æ<?ïú`^9œ.?4›4>@?F~†Årr@?4›4>@?ïïmç«?eG,/?`ä'ã`mÄ?eG,/?îwõº?»û×bŽ%Ù?¯È€°>í?»û×bŽ%Ù?ï>X¦ñW,?—[³ô¨wÈ?˜4ë#Œè?—[³ô¨wÈ?ïÙ¼S¥;?eÁ^ÿ%†?s!Öä]©?eÁ^ÿ%†AGN4FGL J1626.3+3514?í±ïÎ{ðß@Eñ&|k‹iÀ:ý|ªu‰ðÀ<±vö×bR@!)æڕl?öÀ;ú'¾?Ð$þÝ@7~?ÐR9¦j@qŸÝ€y7?þ½ ŸrK¢?ïm­íät‰¿ëU.enâ¿Êj^¼#¿Ê'dÜx'a¿ÞŸxkK¨u¿á´¶á(#‹AGNbll3FGL J1626.1+3512RGB J1626+352?ïðvþ—¨±?W[e|<®µ?_jú.	?W[e|<®µ?ïÅ|'BÌ?‡ó¥cÝ6?}A¾íR?‡ó¥cÝ6?ïƋ™jŽƒ?xCæ®Ó-?|º3H¨úƒ?xCæ®Ó-?ïZ²Ù[¦o?tôþ¶Q$Ô?"©¤ÏcÈ*?tôþ¶Q$Ô?ïç–Šgð?h
:Ð8L°?h=iX»X]?h
:Ð8L°?îÛ
GžÑ?³'s·ž ?¢O[‡æï?³'s·ž ?ï'‹ÓnŽ?XH"¹øï?y$\'?XH"¹øï?íÇ7›'…=?›ͶиÊ?±ÆC#sÖ?›ͶиÊAGN4FGL J1626.4+1820¿ï'd«Ÿ…@DãC0×8À:Œ"¦£mÀ<H'sg@u–Eý`@ÞûB0&?ÂhÁ_†M?ÏáÕ§?ÔM¬[==@ôB‡¿å;¹^Û؃¿Õ~àEO•j¿ì
c›°Ë¿áš«n®4¿à†FÁ—"¿èP%1€¬AGNbcu87GB 162358.1+182615?ïú	Þr‰?CÚËzs?G؅RÏg7?CÚËzs?ïò(䥱€?_âÊȸ+…?[®7š?_âÊȸ+…?ï¼2‰°Õ?«Äân.è?€ó{*úDÌ?«Äân.è?ïõd¼Hh?=9ù§Í?U7æ`ó'?=9ù§Í?ïÙ±©¶"?r®'¤k{?s'+‡R"A?r®'¤k{?ï¶è­[ î?ŒÊÀZ š?'EÔ¤ F|?ŒÊÀZ š?ïGÁ|Pw?"l‹›3Š?—'՝[?"l‹›3Š?ﮇç.fµ?sx½N~5?"^6 Ý?sx½N~5AGN4FGL J1626.6-7639?ïÁ±7'_áÀ2͇+À:Ba¤`À<Rmý3œå@ /ù€_
ý@LÓi©?·b>
¬»à?^ê8§în? ˜‡Üéá—@	xš¶O1ì?×»©äÀ^¿ÊDAùI­¿ãqøjà¿ßŽÞ	àÿ¿àúÓOÍ¿Þž6œLÒAGNbll3FGL J1626.4-7640PKS 1619-765?ïþµLIüñ?í&øœª\?$«7>vS?í&øœª\?ïõgÔ?\@¦&Ýr?UÝÖe¡ø<?\@¦&Ýr?ïø¤§Õ ?;ÑwJrª?Mmduy…í?;ÑwJrª?ïýæ¹?!P·´é?4'»Ü?!P·´é?ïýæ,Å/õ?#Ëó¡¶hC?0ΗË">?#Ëó¡¶hC?ïÓ¿v¼¹ž?–C«ºÿ&?v D¥Â¸õ?–C«ºÿ&?ïøÓQ‡mX?`Ly»ºÏ?L²¹;*lP?`Ly»ºÏ?ïúÃ$ØQ?7)V™—žî?DókÙ鹩?7)V™—žîAGN4FGL J1626.8+4337?ë¤y('L˜@EÿO?Ù3ãÀ:ÏÀXJCñÀ<Š¬®IT@ÀjS†@g@€ù?ÈQ:€Y'?²²"Ç!è?ã±2!»;«@îOá¿£?ï¿}X›M¿êB€x`cî¿ê×¹Z)AB¿à£Ò¢Ï£A¿ïþQ€ž¡¿Ï•½ÁìôàAGNfsrqMG4 J162551+4346?ïܧ1¡|?|`Ð}Åù?q¬gFŸ{?|`Ð}Åù?ïïOîw8é?a"ÇKW'?`°š¥ð?a"ÇKW'?ïÁ©³öš¯?*0kßÍ]?+&"ï8F?*0kßÍ]?ïÚûEÇ?\é—	þ¥È?r']V_³?\é—	þ¥È?ïâY˜ïòä?væøgÙ!?m¦gDG+²?væøgÙ!?ï¾2À"i?á‹ß"l8?€sOõ¸Ç?á‹ß"l8?ï¶0àamó?"ûtÁM0Ã?'sÇøҏ/?"ûtÁM0Ã?îÏiI<+w?'µa!³ß?£	knÐý?'µa!³ßAGN4FGL J1627.3+3148¿ÛK4æUxÇ@EŸå\ËOÀ;
ÿ'E7À<ªmà®+!@ ¨7F=Q?÷º›<1·?Ò×Î]›'–?Ò¹C£Bå®?ôJ…) z@ò‰§ß®¿å—O§Ýÿû¿ÝÔëŸuѓ¿äàNjDlA?¶g¡	$—¿à
¨à"Í¿å¹êqùA AGNbllNVSS J162712+314954?ïõl<­õ
?Q?50ùœ?U'†%¤Lw?Q?50ùœ?ïñIœ‰Á"?a\#'fy?]lÆczô?a\#'fy?ï½$îCav?~=ŒÉë+?€¶Äv^Ðt?~=ŒÉë+?ïð¼!2ù?D
˞‡'?^‡½'c¾]?D
˞‡'?ïôró^ÿ6?Vþ~…Ìõ?W½³'¸?Vþ~…Ìõ?ïÇoñˆ ©?"Ìã3p¹´?|HD.»z?"Ìã3p¹´?ï̅u†{?|OLØA"R?y½E!E•£?|OLØA"R?ïÓ
Åð~r?gIšÿþY?vzœú²CK?gIšÿþYAGN4FGL J1627.3+4758?æ,nÿ£J@EƤ~Ïé¸À:вýî­ÈÀ<™M߆ã´@Ÿ…@ò
¤@Ú`üšò?Ê0HÔÛd?ÏYÌ9©ïÓ@¿<pɖ·@"¹D8¿¿å塄õs¿àÝ6aé¿æbEÚÕ¤¿ëd¯­Uk¿ïð¨ÿ¾Ç¿é	lLþAGNbcuMG4 J162750+4802?ïòƒ¦ÏHc?W·ã¼"y¬?Zø²5t9Ž?W·ã¼"y¬?ï¥VÎeJª?zE?†ªLjñ?zE?ï°ñZIð?vjB\Ošö?ƒÃ¿"ŽL?vjB\Ošö?ï%"FÚb•?~¬Œêu<?›[·+'åQ?~¬Œêu<?ïÛya£Î?påu€®½Í?rC@HþÍ)?påu€®½Í?í™nybõ÷?»¼"3ö@}?³4Œ4iH?»¼"3ö@}?îilfkÖ? {àï@*˜?¯‰i:u)Ÿ? {àï@*˜?èµX³º?±›
÷™˜Ý?Í*1"ß?±›
÷™˜ÝAGN4FGL J1627.4-3301?ßßÃDʊ@%ëßm¹@ÿÀ9ÎÌ¿`ÓÀ;Ž1á#›æ@÷âzÞîb@BVÃ[?Ä¿4žBJÓ?Æ«:ÖÀ–‰@ÒÌ:֕£?öÙ6Âß¹?á¡èˆ6?ïüÀآĿê´k¬÷Dp¿âi`Kš2F¿ð?ïÝüÀ/…AGNbcu1RXS J162725.1-330322?îŒgçð¿›?±*}G4,?§9<8O?±*}G4,?çüUÜ=?Í®…ŒÏå9?ÑúUèG…?Í®…ŒÏå9?홛«}ØÚ?ž:Òjĺ?³3"¢Yk2?ž:Òjĺ?ìZ:>Տ?¦™öþÒíô?½./ö	Sˆ?¦™öþÒíô?â_ó(½I³?Ðìwi^Õ?Û@®…lš?Ðìwi^Õ?Á#_¢õ/?ÈÝ>\å'È?뺷(B´?ÈÝ>\å'È?ä'þÏÜÕ6?¼z'ÅÔyÙ?×°`FU"?¼z'ÅÔyÙ?Ò&?4H\?¼åÚm|ã´?æìàeÛÑø?¼åÚm|ã´MIXED4FGL J1627.7+0251?Ðötª»š@@{ñA [ÀÀ:" ‰ƒœÀ<o§yV-3@F‡"^qO?ýŽö¨hi?Îs€?ÖY¾?Ò"¿µî?ÿäùdŒW@	âe£û
¿å	%B°¿æ…ZýýqZ¿Ó77dENê¿á­š'w¾þ¿äÞ><ü‹¿ïìüLíAGNbcu3FGL J1628.1+0254CLASS J1627+0251?ïú«¡ü6?>0^rt7E?EQxÌÒ!'?>0^rt7E?ïã–+"È?|(X(«ï?lûi¬À%?|(X(«ï?暴jyÙ?'n
8£B?…ÞeP'½Ø?'n
8£B?ïëEþçÒ?H³H"d7Š?dº!ÌÜ"?H³H"d7Š?ïø$ç•ûÕ?Nƒ"aê³?Olbxl,Ú?Nƒ"aê³?ïhÃÞf¨+?¡h3:×ý?'ç"3*ú«?¡h3:×ý?ïg$>bM?n¤R¤?"mø3¶n?n¤R¤?ïÃÀm²¤Ç?h
Í­Ñ>¶?~É6{ÐN?h
Í­Ñ>¶AGN4FGL J1628.3-3343?é0Η'Ny@$±·|¯ÞÀ:ê#èùÀ;âo¼h@ Y¶Âs@Õþ¤¶-N?¾«>‡¥%i?';|¾þ"+?ÖÊû>ÊÁ@.d,$v?ïþÙú²¹%¿ëb†÷¿â‡k>gnÏ¿Þ1œDÄ«¿áP·b­IO¿ÓW<½J£½AGNbcu3FGL J1628.1-3344NVSS J162819-334342?ïî8ùòÅ?mÛÑàým>?aÇ|­bí?mÛÑàým>?ïØ«ùèö?¨ï£="©?sªv›Èï?¨ï£="©?ïÚ­Tr¯?vžm®¤+»?rü©AØì"?vžm®¤+»?ïò=Ù·i?CB‡|`'?["M\ .$?CB‡|`'?ï߉`øyŠ?qgr
ψß?p;O‡2Öð?qgr
ψß?î֓D7^Þ?¯óÞÜRi?¢–˾Aà?¯óÞÜRi?òÄqù?Œ:Æ7N¤?Š™ÃY2U¦?Œ:Æ7N¤?ïÃÅûÞnq?mMz	?~
Y+?mMz	AGN4FGL J1628.6+7706¿î#Пó®l@A
[–(ËÑÀ9¤š~›çÀ<,žZÉz2@H¼áGX.?ÿS‡œAÇ?¬ß¾¥Ð?·mÅÖ8†Y@
Ý®ˆ*Ü@…í
´ôi?ãþC›`C¿×û=j¿à8@¹-³—¿á­ýžü¯é¿ä"q`¿åò"šCäAGNbll3FGL J1628.2+77036C B163030.4+771303?ïþDAV<? A¶Fz‰?+»ìÏ|w›? A¶Fz‰?ïöҜðf/?TvJQc'?RZŦAb–?TvJQc'?ïìFy$óÄ?b¤
´ö Á?c¹†Å»ý?b¤
´ö Á?ïþ.¿c¶?ùª`ô/?&ý
@´z?ùª`ô/?ïþ˜I7w?¯³ýÓ¦}?&{i%~O?¯³ýÓ¦}?ïÕÅþ–Z?yÐ4géá?uwÓ?yÐ4géá?ï՜Šöϼ?B#"^ÿ?u1º¡tÙð?B#"^ÿ?ïý˜gs	k?#dО?3<Å݊)M?#dОAGN4FGL J1628.8-6149?ãÖßȼÀ"a'ÚÀ9Z귙^áÀ;³ÙésÍ@Ÿ¸7"kÝ@Æ[ê¡õ?µ›ƒ~¥!?Ϫw¢Î́@"ƃÝ@ã&q÷?Íî´(;2†¿ãf…·æ¿é|¢èÍ´¿èÝíPÐÒì¿ì̦×o½þ¿ïý9Fr«AGNfsrq2FGL J1629.6-6141LQAC 247-061?ï"ÞqÃo_?ªf<g¾?ŽÈc}öt?ªf<g¾?ïË­M*«$?Šd÷q(F?z)YHþB?Šd÷q(F?ïB 8š%?'N²zÙ>?×«ò
ƒ^?'N²zÙ>?ïÙò\?Y"›¤Aƒ?st†ã%()?Y"›¤Aƒ?ï'ÿ÷q'?œtã:Œ<?íŸûêcå?œtã:Œ<?î˜0Ó(þÉ?´³7rA—Î?¦|òÊwq?´³7rA—Î?ì:ԓPæ^?¨EÊ@~Á?¾)[exÍ?¨EÊ@~Á?îM~ã8Z?•‰)•íÀø?«(õ<W?•‰)•íÀøAGN4FGL J1630.6+8234¿írUB°1i@?:kÆ!·áÀ9
¸ª*À<&VÁ­´Ú@Îæcæ"@²>¬
:?¥ž»AŠ?¶Ì`@\'{@%äêÐÄ?ýTâƒBj¿±yƒÿæ¿ß^謿ä¥/š!~Ö¿æB• Ž¿êÛíÒt¿ç
'Kº"AGNrdg3FGL J1630.6+8232NGC 6251?ïc0ßEö.?Sԃôm…?"™äў7?Sԃôm…?çÙ?#¬WŒ?Ņ)%¤eŒ?ÐM¸§Pç?Ņ)%¤eŒ?í7¹¸¦'¿?£}ÂTwX?¶B2<Ĉ?£}ÂTwX?ç'~ΣLÝ?±eNz´?Ðûb¹fF?±eNz´?éØ
%é"Ð?ÁZ©Fcz?ȟËhYìÂ?ÁZ©Fcz?ȼ[R-–´?ÅxÐK?éÐé+tšS?ÅxÐK?茪ô'?±.Uc?ݔ?ÏñÍWŒ-ö?±.Uc?ݔ?Ë,O<0æZ?¶•à±Ãøa?é4ì0óÆi?¶•à±ÃøaMIXED4FGL J1630.7+5221?Òd‹?Ž¶<@E2\'ÑN<À96Jbú¡À<Ãõ¶7@G¶¶_øä?ÿ%"Ùîô??¨ø%
?Ž?¯Tkì @Oäë8@	l,¨T¿ÔzÁWÁ¿ÞÚÙÕÊ¿á*p·"@¿Þµ6˅…¿áÝù ?{¿æO6WªâAGNbll3FGL J1630.7+5222TXS 1629+524?ïþ,('?">êaV?-=yËÊéî?">êaV?ïï·ÐÖ?eä@53m?`æGô­ª?eä@53m?ïïíWu¡‡?jʵڐ¯c?`¨¶Yy1?jʵڐ¯c?ïÕÍ0Â7?YŒ!Ö#k ?ug"ý?YŒ!Ö#k ?ïüeþ ?5îß©Rk¼?<×è?­TÜ?5îß©Rk¼?ïÊð´ç'?y4z'YÄÃ?z‡¥¬Ÿt?y4z'YÄÃ?ïâÅ.jC?w¼v"²0^?m:Ñ®z#¢?w¼v"²0^?ï_s))?zýasÍm?"LQšÚë?zýasÍmAGN4FGL J1631.0-5302?ëª[™êÞÀ	ú D®…ºÀ9›)"N>À;3+­,ô@
fÑ@OÙâ_I?ÉÏìçÊT"?Ç¡¼}Ê0:?ÿÃ¥¦î?þ,iˆïú?ï—c"$ӿ犻°DÖÊ¿æÄS­úпëoÖ½—'¿É¥ì8Lø¿ïÿxáh:QAGNbcuPMN J1631-5256?ïå"Ä{§?gk/à®?jÝ;bŠAk?gk/à®?ï#ìÿиÈ?¨t51?›'`	X'ô?¨t51?ïzûV÷?›Ì²rCï?Ÿ ¤4Y!?›Ì²rCï?ï¨ÒG—Ä?qÅÙS]V?…Ë~\ì
?qÅÙS]V?ïC£-?˜j¼¾…ä?—œlKœzc?˜j¼¾…ä?è͌Žªc}?Ê5HóJ ?ÌÉÍÅVr?Ê5HóJ ?énzÃ%ë?²®¯Åè?Ë®FóhS?²®¯Åè?êè'=‰ø?µÁ÷p_D¦?Ä_cØ!?µÁ÷p_D¦AGN4FGL J1631.2+4926?ÝÓû8€@E`GýœÀ;$›À»GÀ<¨a¦
Ec@O+†®@ëU¹oø¶?ÉÀˆÊ>}?¿à¤ø?òéÆؗ?øµñ–°±
?ï*u¿á+3Šq¿í'ÿò> ¿Ç×ϊAaõ¿ïî¡UЗ¿ê;+ðHÒØAGNfsrqTXS 1629+495?ïðSYH?_èZ¤À¯?_éYÀN°Û?_èZ¤À¯?ï!îŸ&î¤? j_†'£y?›Â,²? j_†'£y?ïr͎$?…¨R¦i•?Œ#LŸæ›È?…¨R¦i•?¾ž?ÎÓòŒÎ%?§†DÖF?ÎÓòŒÎ%?ïfýÈ×ö?–´'_2˜î?" _ÊTG?–´'_2˜î?ê1Ñ\:?Çq›ó)ò‡?Ç9Ã캏?Çq›ó)ò‡?ïaŠò?"' 9ãÿÙ?œs썥Ë?"' 9ãÿÙ?åÄPÝ?H?º0 '}.?Ôw^Eہq?º0 '}.AGN4FGL J1631.2+1046?ÌU®÷éu@Aü¸{Üð0À9ÌöÕ´ÒÛÀ<&ç­"ãZ@0&îV_]@->" 
Q?¹ñ:j_k?Á!Í°!›@^¡£SW@ÿ³ÿÌT?ïýZž²O¿à‰xïÕæQ¿çYߥ¥^¿â-¸j?8û¿í;‰]â3f¿Õ:Ûs-ÊAGNbcu3FGL J1630.8+1047MG1 J163119+1051?ïõð0˜èÞ?RAŠ"Rç?Tžñê2ú?RAŠ"Rç?ïãkjÉj?wäÙ"=?l"•xu¦+?wäÙ"=?ïœr<'"?‡Ô¸'qûó?ˆãpæ²î?‡Ô¸'qûó?崙ü^¾Z?jiÍôt?†€áq1Œ?jiÍôt?ïÍë«è¯4?|ƒkñÉé?y
*#½Ö?|ƒkñÉé?ï"t‰?":ˆ0{§?¼år6Þ?":ˆ0{§?îæÖBŽ½??™d÷q(EË?¡'›Ó¤?™d÷q(EË?î4©à08?"ÆQwZÄ6?¬µbø{?"ÆQwZÄ6AGN4FGL J1632.2+0854?êó·K–@AuT\x¦ÛÀ:7,ÅÇÀ<Eq±ôr@qjKÎ4¬@*"³‰.è?ºæPA
$?"'CoÏ?Ûå'`À48@
X!þ­o¿¾63Úg?¿è(ÝnÛî¿ä+3Šq¿ãg&f¿R¿éïm«Õ€?Œò"‡$çAGNbcuNVSS J163211+085608?ïúÄwœLZ?<,ӂjä£?Dî!˜³Þ_?<,ӂjä£?ï¬ú?pe?s€#Ö?af~Í+ˆ?pe?s€#Ö?ïå‹Q¤¯Å?j~!mX?jt®ËÛ*?j~!mX?ï÷þÚÑ?9©"å˜?Pø"n¯
?9©"å˜?ïç¯!Úà?`]Iøí +?häPԆ8?`]Iøí +?溜~ñ*?O±†?† J˜í‡?O±†?ïÕÏG{i®?|°0[%ä@?u\Hzu?|°0[%ä@?ïäyH/2Œ?XL=6<‹?k†¸
†ãR?XL=6<‹AGN4FGL J1632.4+5800?ï!÷Ø@Dzl <K
À;Ҙö«;À=µ?è@ Æ*ÚI7,?ýPaâs'??ÑEZ}$
?±‰Ä6Š?âi¿aTXÈ@Hñ0.q¿æ7­wa¿î-Ƭø/¿ÃÚÓÍ$á¿ã@9¿Ü0Ý£3Ì5?"gâèB3AGNbcu1RXS J163213.2+580109?ïþû§Åp&?Ôä»>>? E'"	‹?Ôä»>>?ïöéÞ-•?UÓay<7?R-ö	ëfð?UÓay<7?ïå4Òð}V?u‡m'ôki?jË,ïæB?u‡m'ôki?ïýMÃ? :³#ÉÆ?4•s/aN? :³#ÉÆ?ïþð…†»? ÔE‰nu¡? ÷§Ø¡
'? ÔE‰nu¡?ïÝÑBJË?rÐ-ýÛ·È?qzR|Á?rÐ-ýÛ·È?ïï¾ÖXÖu?tlQ|k;?`A)N‡?tlQ|k;?ïõـ0ß=?JX±Š©¢?TLÿY‰U¡?JX±Š©¢AGN4FGL J1632.8-1048?㣃‡«Ó@8Mqâ›k+À9Ï0âöÚ½À;ÆQ°Ì¼@),P•ï–@Z䢬gÒ?ÂʌU¹E?Àɽ£ºò?úTâ_ܪ@"šÞ=7™?ﯷjdù¿âº¾ý×0Ô¿è';2ô¿å¶<'gN¿îŸ™Þb÷F¿ïö±½|ͱAGNbcuTXS 1630-107?ïîÏٜ"õ?iÓ67Q×?a0&NÎc3?iÓ67Q×?ïâ]Ȉ"?x"'ÁõÞ?m¢7–"ûZ?x"'ÁõÞ?ï#"Ôûð?"Ø"ç¢?›Ÿ`9ý?"Ø"ç¢?ïü¦ž‡6?'dËôš")?:ËŒk¢?'dËôš")?ïêœu/ñ¤?k^•á ?ec‹f³—?k^•á ?ïR£å31A?¡z<Š‰*?•«ƒ]	sÜ?¡z<Š‰*?îGþ<9ã?¢‹l°¨5?«€<nÎ?¢‹l°¨5?ï÷±w†Ê?BpÍ­
÷?QМŠA¼S?BpÍ­
÷AGN4FGL J1633.8+0701¿æÆK×w~D@@Ú4üaÀ:>*ՖŸêÀ<QÑææT@<~"ÛH@½'Óh'?¿XÊ`OºÂ?¶ÿ¬ž6?÷vÙ˸З@	'øŒn7ì?ïŽ!ÛòÚ¿º½¿~/°È¿à©(ü¯i¿ánÄÙ¹D¿ä÷K[H%3¿êÇ/~ó¦AGNbcuNVSS J163350+065705?ïüôŽÌzÜ?+dµ–?8[‹nZ'o?+dµ–?ïè¡qª<T?p¦W•W³x?g^Ž"œ£'?p¦W•W³x?ï:?b)='}?ajGð¥17?b)='}?ïØ£¾œÄƒ?UOî\kõ?s® ¥?&Ë?UOî\kõ?ï÷Й`
Ý?J%ËG?P^Í/¬…?J%ËG?ï'3ÿv?™ÛjK,·	?‹¿³
ýÒP?™ÛjK,·	?ïæñÚ+Ò?tÀiU:÷?i%˜z¬?tÀiU:÷?ïŽþg›çõ?t¶}n*?Œ@fužÁ?t¶}n*AGN4FGL J1634.9+1222¿ì…û'ñ@Aé4?¢­?À:øÓêÎ?"À<dInÞÛ@ #4ÔžÓ@(ã«5£?»­¢e6¿¸>Ú 
ëÀ@‰2"Ѽ?ûž"Ør}?ïûlb&¿è¢µ6®÷¿ã #Uož¿îû9Ç¡ê¡?âòc"úÎh¿ðAGNbcuNVSS J163502+122142?ïÜî!ls?£ûEpÀï?qû‰
Ʀš?£ûEpÀï?N†JÝ?ªFìr‹a?Ú¬P®ØÁ?ªFìr‹a?ï2'SšË?"\ßD—¶?™»ŠîÀn?"\ßD—¶?ïë*CS‹?_@‡PÞ?dÕ¼¯¦$Ý?_@‡PÞ?ïÏw¼Ïÿ‡?ƒySD÷Þû?xD!®­¨F?ƒySD÷Þû?ëh'"ٟ?ÈÉ*ù^?Â_"ct™…?ÈÉ*ù^?ʊ°Ñ?žÀ]ô??¦ö£SåVó?žÀ]ô??îƒÚeÅ4[?§vcËïg?§ÂY =Z?§vcËïgAGN4FGL J1635.2+3808¿ÅbÃLNé@E*â:¸cÀ6K¯*ûVÀ;	ÇÿÞr@Ÿæè%@£$\֚¬?"}Y"M?ÀMfûŒ¨Å@4 uĨ;@!›fçÀ™¿ÉTå ig¿át·AË&"¿ælÐxR÷õ¿çP¼ R;¿ë·
è`Ý¿ïÿõïùAGNFSRQ3FGL J1635.2+38094C +38.41?ïu$œía?ªûÓÒMàÌ?'[l`œ$?ªûÓÒMàÌ?ÈrāzÝ?͂ÿ"Úñ?éãNß¿¡I?͂ÿ"Úñ?쎬_]ÍT?¨Ã›'ñsp?»Š•\?¨Ã›'ñsp?Þ;‰L´'~?Ò¸N{
<?àâ;Y¥ìA?Ò¸N{
<?ïXjIõÂd?"U@—V+?"ò¶Ä·On?"U@—V+?¯«â,Á??À28»¢ã?îAÝ3æü?À28»¢ã?³¦w? \	%¤œ…?§UÄÎ=ʘ? \	%¤œ…?,A'X?‹Î³¼6zÜ?ïÁѧäY?‹Î³¼6zÜMIXED4FGL J1635.6+3500?î–ˆB.N@Dü¼œÓà½À<¦-%ÒøÀ='ž>Dn@Õ³¦53@÷C˜Ü?Údò=I·"?ï*~ŸBP@.ðþÛ<Ò@Çy–™ßæ¿ïqÞ?ïýnŠø'¿Á‹½ãÐÊ]¿ãàâΖÑh¿ïÿx@XŠ±?å(@[9âzAGNbcuMG2 J163505+3458?ïz•ET¦~?—íEûþ6Ô?­WZ'š7?—íEûþ6Ô?îRüÕå5‹?³¹‰gtÕ?ªÐ2£duU?³¹‰gtÕ?ì—
h•¸?¤¶3¡Jƀ?»G÷"»R@?¤¶3¡Jƀ?ëü ËÉm?¥v#º´?À¤ÐÚN?¥v#º´?ìýÚþ,¯û?ÂŽ ÊÃç?¸(vg&?ÂŽ ÊÃç?å´}¹Fæ¢?Ò}€§?ԗr2¼?Ò}€§?èW˜‹ã´¬?¶Fh¬'?ÿ?ѝÐq-P?¶Fh¬'?ÿ?ÞvY6ÒU?½±|©Âö?àÄÓdý–Õ?½±|©ÂöMIXED4FGL J1635.6+3628¿åÅRó ~Ä@E"î9.À: á$r¦À<	t"&"@wæ£ãt"@ë&T' ?º0@åxjJ¿ªµèž~I¡?ënþ…¬|Ë@ªÖÍvì¿æM˜9GIk¿åcÉ2äXÛ¿æÞ£ßm¹A¿äõ'ÊIdοïÿö$´ë/?îï'Á8AGNfsrqMG3 J163554+3629?ïýI-Š@¥?0·ÉhFŸ?5¶"ÅÑ¥?0·ÉhFŸ?ïõm¨$!?Zó«'d`?Uõ$U›?Zó«'d`?ïØrÿ•»­?vÞg•—¬²?sƀ-"^?vÞg•—¬²?ïÿ´¸{S€>öئ®t²n?ÑÜá_mÍ>öئ®t²n?ïüä,Ã`?@&'ÛiËú?8ޛh†'?@&'ÛiËú?ïÔ¡üOØl?yŠž»%é?u¯éAÖ?yŠž»%é?ï¾fTj1ï?ƒåE6¼dÖ?€fjßô$0?ƒåE6¼dÖ?ïþŽa	ã·?#UãI%â?'óbƒ;*?#UãI%âAGN4FGL J1636.3+7128¿ï|ÛÆí"@BbA=·ñÀ:ê‰Ê½fÀ<šlvJà@G`Ö@r$'–GÖ?»ÆUˎ‰¿¾4b2O2˜?ýûk{y"@•àZôi?ïøf–=ï¿ç_·ö{ó¿ëô(üxŒ¿á;Þ}yR|¿á@W¥ÙC¿ïÿèã«6AGNbcu7C 1636+7134?ïê¥W_YÏ?œ#‰C¡o›?eZ¨á>؆?œ#‰C¡o›?ïÜñ,JO?uLul?q‡i`?uLul?璉[c [?ƒóš,k·Â?†Zé'éM?ƒóš,k·Â?ïۓ"ûWØ?^Ù³ÔÉh?r65f×4?^Ù³ÔÉh?ïÜåÜhKC?r¬QºÚGd?qêî\?r¬QºÚGd?îâq ðê¨?§ûžúµ?¡Øåó…
{?§ûžúµ?ï}¯¥–õ?"ü&öq³b?J%·^?"ü&öq³b?íêŒéæk¸?¡D+eíË?°«˜®¦àÄ?¡D+eíËAGN4FGL J1636.5-0454?Ô_Àá:@:óúã`	À;"ˆ\ÙöÀ<XùD$?@!ñ¨Ôõæ?ü—ù1~'?Ó3®BÈý_?¨$ j»'?Ñ» |ø#@G6·!>ê¿å›¥"
ñÛ¿íàœ…˜?ÅYGŸœ¾¿æhãï(Ah¿ÑßÇ[Ýá¿Ï…òGۋ×AGNbcuNVSS J163631-045506?ïýŠ
k¤û?)öDnRéá?3¯®r?)öDnRéá?ïßpòäí?€w£v!ze?psG™ËYa?€w£v!ze?ïÔøpé]?w€{¼j#<?uƒý9Ìáb?w€{¼j#<?ïóò‡‹=û?DV*$/ûì?Xðô'Éø?DV*$/ûì?ïüìN¿£?5Ö'm1i?8Œ(¨üÊ?5Ö'm1i?ï:uàÜ#?£ u‡¿È?˜±\{Mu¡?£ u‡¿È?ï˚
‹Qá?'	"è=?z2úؓŸn?'	"è=?ïʈ°íö?qØ,ñ2"M?z»§Ý;qQ?qØ,ñ2"MAGN4FGL J1636.7+2627¿Ðg™öÐp4@DŒÁDŽÀ:Q÷·\"@À<§".Î@âPÑQl@ÉuDO»)?¾i®oišM?¹
·ß»øû?ûŠYUëÒ?ùgÐáÚP?ïþ˜â9›'¿Þ†#3‹É¿ã<b0÷š¿âgpÛs¿á³´,ÂÖª¿ïëÿÝÆDHAGNbll3FGL J1636.7+2624NVSS J163651+262657?ïð™«7PÏ?V2sX[ó†?^Ì©
mbl?V2sX[ó†?ï·îL? Dô˜ò?‰87«? Dô˜ò?ï®._ 	Ü?'#~ï¡)?"th!ôfÛ?'#~ï¡)?í¸n¥?"hþGùQ?²?"Y?[?"hþGùQ?ï¢ÖÂw'å?†3À§H°?‡JOe‹"?†3À§H°?éÏ8ؗ8õ?ÉÀ3&˜?ÈÝ£-?ÉÀ3&˜?ïp0X|2?•Y´MæB?ùö¨GÅ?•Y´MæB?åŽPéZ)Ë?²b:wi%Û?Ôã^-K¬k?²b:wi%ÛAGN4FGL J1636.9-4103¿ìBlÚ|ki@€ÙÃUTÆÀ9zþ‡YûõÀ;)'o(¬Ç@{1ÊÓMo@Æۙj?ÈWÔþ©c?Ètè_Op×@òyÝ;¯Ù@ÊsѳçN?ïÿÖyô¸¤¿Ã¸«Ãã¿èùD$>û¿ä?˂þž¿ç|éàƒãпïúšï°AGNbcuPMN J1636-4101?ïÎŊÁÃ?vÓ>1/0?xþ(Á&"?vÓ>1/0?îðÍmº U?£ƒ:Ÿ›…? ó)$]ú©?£ƒ:Ÿ›…?ïBïŽ÷1Ù?ŒkDWÙì×?—¢aöé?ŒkDWÙì×?ï'=0."^?}Ø5ë-7×?›Yõ*P?}Ø5ë-7×?ïQ`|0kò?–´ŒW{b?•Óð}b°?–´ŒW{b?è§6ŸŠ†?È÷B'ÝÎä?Íc·%Õê?È÷B'ÝÎä?êk\ßí?°¸YŒ"?ǒRŒƒ M?°¸YŒ"?瞬(—?µ÷ÚÃÍ£ ?Ч¯ÜÑþ?µ÷ÚÃÍ£ AGN4FGL J1637.1+1316?Çóàυ†4@AÚ!xöŒÀ:úmPes!À<sÝo²?ƒ@SØæ
¶@u ÝD?Î4rÎSµŠ?¸"éclâ?îD½¿h¶"?üÛr<2‹C?ï³hëÒ¿áúóPÅr¿ä&Iàô¡þ¿Ö놡D]Ó¿êàˆ!ö¿ïÿý`éNäAGNbll3FGL J1637.1+13141RXS J163717.1+131418?ïÁóÛ.`?­în_¾ˆe?`y@I?­în_¾ˆe?𥉉>.þŠ?ˆ°Kî³)ø?…°{•x?ˆ°Kî³)ø?ïdGK¡?Žâ'|†ó¬?"|³6d?Žâ'|†ó¬?ïl«?~¬IŽX6½?^'xV*?~¬IŽX6½?ïÌÔ°'$™?rUõp~?y•§ÀM‹m?rUõp~?îóÀEn¹?·²ø°åÂ?¯@ÃúÍ-s?·²ø°åÂ?ï7z6–®Ç?"QÃx,ë?™¹.áõ?"QÃx,ë?ë0NHÚ±´?§¤ÚD£€Ë?Ã>Æܕ9/?§¤ÚD£€ËAGN4FGL J1637.2+4327?å¡+§ß¾¨@E
ÆûÒsÖÀ;ÙPVY¨éÀ=y_gn¤@!'ïCš3?õA³(¶Ø?â`€É>"?Þ´Ù% £y?ý	µU·Âz?ìsö™Ïտߝf'Ú?ì8ŸÎz¿Ø"€ð«N?µÊ£QÔ3¿ÝÜ°Úþ¾·¿å95Á-sAGNbll1RXS J163711.1+432548?ïïƒÀig?bgÛÉ!?`ì|FuÐÕ?bgÛÉ!?í9°ëšÃ:?¼>c¬¼?¶2x£—Ù­?¼>c¬¼?ï{絏?"ù/ùDù?Ÿþ™²&?"ù/ùDù?íçÑ©*$?–†S%g?°Ár·P»d?–†S%g?j@Š0?†"/å&ß?€oîv©ù?†"/å&ß?æ)tì>?Ò$‡ÃG+Ò?Óõ­à'"?Ò$‡ÃG+Ò?ï?ò©4?'ᯁ<Â?˜¾ŠÙ|!?'ᯁ<Â?è7Ès?¸X¿ŒX¥?ϟ#—ðÞ5?¸X¿ŒX¥AGN4FGL J1637.6+4548¿æ7£Eûóè@Dý\B 6À;©%ʔä(À<ùZ'ó+@!¯…>BÜ?þ¡YKË°m?Ëz©u¯°?OöìˆZÖ?«¾œ!M€@~3ˆ˜•c¿ïÿT•Ð·?ïÉL¯Ûû>¿ãÆ'+½óì¿éC•ìeïH?ÔÉJ àuK¿ÛÈ…3[!AGNbllB3 1635+458?ï³^•rԚ?´¯µ¢Íe?ƒ(Z'͖?´¯µ¢Íe?ïõêHÄÑ?V&÷r•%?T+mï­.š?V&÷r•%?ïß_flñp?v¬qí²?pPLâDwæ?v¬qí²?ïþº'%*S?'`œ9E?$]Å‹=@?'`œ9E?ïýï÷k©>?=ÌûÈIúb?0€E"p€?=ÌûÈIúb?ïÒ8
wA?xœˆWÄ	t?vãú¯Á˨?xœˆWÄ	t?ïו-å
?}*ìåácº?t5pw{Õk?}*ìåácº?ïø™q€ Ï?KÛX&~sÒ?Mš:UrÂz?KÛX&~sÒAGN4FGL J1637.7+4717¿Ø<Ý\x7/@DðÀƒn˜À8Þ©°â‹À<Aæh2ï@LtQ‹è@,Âþí±I?¢RFýHY?¬&|w"@¦#×þ@¹Ûÿð'¿ÂGpÂ_ág¿äv‹AèÜ¿æ8o'Á¿åM
švX¿è!£=Ý0G¿ëZA"õÆAGNfsrq3FGL J1637.7+47154C +47.44?ïþÜt¾ •?ܱDa?"8´÷ª¹?ܱDa?ïõ¸QÑÀ
?Z!ë­?T\YÀ6L?Z!ë­?ïì½å˘½?mÕ£ur–?cBka?mÕ£ur–?ïÿy°9'?îøì×ê?Éÿ^RN?îøì×ê?ïþ›¢™ƒ°?¥Ÿå\N?&E×Lwř?¥Ÿå\N?ïÕîÜÂ
V?OØê@â?u'¢hðæ?OØê@â?ïâ^¤¡Ä?q³ßÓÖ$'?m¡[¦å¨?q³ßÓÖ$'?ïÿH`¬F?剹 Û§?óû~ôü?剹 Û§AGN4FGL J1637.7+7326?æ;èʕv@Aœa|ÚQÀ;»`iÍ#4À= á÷×=@ ÐåZ7Y?ú̓ÜÁ6—?Ñ&Ÿ|¶¨?ÌßI¼ŒÂ?ùñÅû!sî@g°'£#¿î@5¯å5y?ïÛù%k¼¿á2:DŸlA?Ää^ú6gp¿é–Š ØR<?—çCp˜AGNbll3FGL J1637.8+7325RX J1637.9+7326?ïývyó¥Ã?0ð2
üØË?4L2M3»Þ?0ð2
üØË?ïö¼¢¢'?RÛøs¢™²?R‡îõ"?RÛøs¢™²?ï³{6ñÈ?ƒ…÷CJ"í?ƒ<!9"ÅÚ?ƒ…÷CJ"í?ïûìºÓÐø?*(W«ßš?@M¶k+c?*(W«ßš?ïü¸óQû?6²v,ç*2?:8f/ßöc?6²v,ç*2?ïØ?³¸îb?t1yt¶
i?sà&.‡Ž¿?t1yt¶
i?ïyzÞ€\?{¿uª?Ð¬K,u?{¿uª?ïô9\†Ø?QUºuÊðô?Wٍxl®ð?QUºuÊðôAGN4FGL J1637.8-3449?Øh…íaº'@ L׌CoÁÀ8ì=áâßÀ;²ïQ/@ h½1øv?ý"
¹&&Û?°?lÒf>Î?³a(c÷KQ@¹üȽ@ŠT©$¦þ?ïìæè×ÅN¿ã2´ˆ2i	¿ÜÀþè(¿ÕN]Ƅ´/¿à¾há?öe¿à2ö—¡qÕAGNbll3FGL J1637.6-3449NVSS J163750-344915?ïýÜ<½‡?:!˜‰C7Š?3ÖÒ%3?:!˜‰C7Š?ï¿®6Љ?‡µlÍ¢y?€r€‹¶?‡µlÍ¢y?ïé†ë°×h?rN=-eœp?fyPˆp_?rN=-eœp?ïŀ¿Ð\q?fdr8Lº?}? š?fdr8Lº?ïûð¶ù&?:|šÃ*Û£?@?èeW«?:|šÃ*Û£?í'¦'­'?½§Edõ3Z?±ëjÊ2Åx?½§Edõ3Z?ïͪ·›…?l7¿""õ?yp*¤2=¯?l7¿""õ?ï61†Fí?‡/hP#H?™9Ï0^ªv?‡/hP#HAGN4FGL J1638.0+0042¿Ö¹3<îH@=¦ë¢zé«À;-¸éÀ<‰¿1×@"(Z)ÂC?úTœ×%?Ìvì…ú«W?©T"¢Í±
?àÖJ>ès@]/Ûæ¿é««Ÿ«y?ïÿY²"ý[¿èöÝÂhp?¯p
BèÌ¡¿ä
Cë[r¿Æ¨Ã
†AGNbcuNVSS J163809+004223?ïýŒË¿?*s3#£c?3ŸZÿ¬Ý?*s3#£c?ïÓõtz•?'˜b†`Ãk?vE҃®=?'˜b†`Ãk?ïÚ×+9Y?t‡An߂™?ró"UÅ«Ý?t‡An߂™?ïâæþëòœ?WÔ _?m(«6?WÔ _?ïý¹É\LT?-'…ó;¾7?21´Ý××#?-'…ó;¾7?ï1P#ƒé?¤YaÄóœ?™Ý5þÿæ?¤YaÄóœ?ïޓî¬=?ws°Uºþ?p¶´0S?ws°Uºþ?ïÀšdoÁ?"ò"ë0¦k?ìµ)ÕØ?"ò"ë0¦kAGN4FGL J1638.1+5721?Ñ;
Õ=@D/ŽèÀ9Í|ÉV À<†ŸJ³'y@;Y:Æ@Ü6r?±¦îýàQJ?³
è³³ ?übÏØðÇ~@°ŠÖ2Q6?ÑÓ-äê¥Ñ¿çßÂ=&Ñü¿æôV2ì¿ë
`¬B"¿ãæò}`}ï¿ïÿ7J³AGNfsrq3FGL J1637.9+5719OS 562?ïþ±&[¼ó?{ßóŏÂ?$휠ì?{ßóŏÂ?ïö#–ˆ?Xm­l[ß?Sý¸‹wñí?Xm­l[ß?ïðԌg_"?VÀŠy·F?^VçCYœ?VÀŠy·F?ïûÏÐý®?-èôÖî¤?@Àò¡Õ?-èôÖî¤?ïÿ>!bŸ?µÜ½a¯¸?;Ӝèµ?µÜ½a¯¸?ï܃>–ò(?t
v´´÷r?q¾`¸¦sø?t
v´´÷r?ïçÎÖgUO?j´Ø@™?h1)Üç?j´Ø@™?ïñq—ûgs?M.5—Ž?]ÏÄxëN?M.5—ŽAGN4FGL J1639.2+4129¿îhg£Zì@D܁Ü
²pÀ:^þُRïÀ<HKv @õõ0Ä@ˆœä§´å?ÃDuû°?Ðìà=—æ@
ί%@8у?ïþ@bEÅ\¿Ý݅íjñ¿âÁ}
q؊¿é!¿îB¿ëK¿Ê߀ƒž¸AGNfsrq3FGL J1639.8+4125MG4 J163918+4127?ïèltŒ2Ã?b8…ò6­€?g"‹o­µw?b8…ò6­€?ïï·kø²À?bª–(ñ?`H",x
?bª–(ñ?ïlò~"Œº?†êÀ0dÕJ?'a°+þÌÔ?†êÀ0dÕJ?ïílŽJþ?Fä4Œ¶r?b"ônõQ¶?Fä4Œ¶r?ï·a¥%WÂ?ƒ ýѨ…?''–ÁPÙi?ƒ ýѨ…?ïÆãàÉ?|~þ/"Ç?|þú«¥?|~þ/"Ç?ìµçò>?¬Þ­7ð­?¿zPÇ n?¬Þ­7ð­?ï­a#ÜS?p/¿Ô$‰?"¿çÁW¿(?p/¿Ô$‰AGN4FGL J1640.2+0629¿Üü͟ÊO@@*Ã") À:º$§5jÀ<f®ITè@!P5©/8Ó?ý}<9Aj?¿Ž9ø¹¿r2byíŽ?´; C¦7@ùùü/æÍ¿èÈEßÞ"?êBÀh Ó¿åù#7<­/¿Þº/(¸¿ÖoïœZ" ¿Ô1"\p™EAGNbcuNVSS J164011+062827?ïû‹
N|T?;¯z¥?AÓ։•'¶?;¯z¥?ïè¾þ¶‡o?v\ræ2>¹?gA\¶a>?v\ræ2>¹?ïçÅ;;ž?h©BŠ8Z"?hã;]	¸?h©BŠ8Z"?ïêàf»("?P ‡x"?e™y|"?P ‡x"?ïôK!͖]?PÒ5rú²²?Wi»Þ"—¨?PÒ5rú²²?ï˜Í¹(L?"Ÿ9_ªÜù?‰Ì'²}<Ø?"Ÿ9_ªÜù?ïã}Ýó³
?s٪̶î9?l'"K²ñ?s٪̶î9?ï©N$ry?všñÙܵº?…¬væÈ=Ê?všñÙܵºAGN4FGL J1640.3+6850?ï¶oªÕ"©@BgNe¾ ºÀ:ÃfÓ'ºÀ<ō²Û‰ÿ@(j[i@PÒÆÒí?¹Ö°™†¿ %üCÕ9?åƒí€ ¡¶@š¥'Ÿz.?ï¦Eÿ¾'¡¿ãxK é'¿åMåр´¿á¬4Á
!¿ÜÈ+'¢"¿ÝmHmWpAGNbcuNVSS J164014+685231?ïþãiI?!j¤ I¹??#Å̝š¿m?!j¤ I¹??ïöh"MÖ?Wg¢+†'?S.÷Œ+ƒz?Wg¢+†'?ïøì<°F?avFÅïˆ?LOÒÿ€y?avFÅïˆ?ïýv—M?"XÎÁf§?7œKs—ü?"XÎÁf§?ïþLU²Ô?&å…XÏ?.;;÷yå?&å…XÏ?ïÙvÜUUó?x€{{Îd?sD'Ö´Þ–?x€{{Îd?ïü¾që)Ú?Bµ-ܚE?:o—Ý}?Bµ-ܚE?ï÷<ž°žˆ?>~ míõ	?Q†ÂD
A ?>~ míõ	AGN4FGL J1640.4+3945?ë¾7fÚ»´@D¶¸ºÇÀ8T¢eðõ¡À;r:?–îÄ@àðÎ^È@ ðÀÇÛÌ?§É·n–¶?®ùQ~ç€q@ÂÈ>Ȓ«@úÕOӿܤ–LÝÿ$¿æz8«B8Š¿åÜ7£Û<¿å3"6‹­H¿çþŒ}Qdw¿ï>ÎÝHEAGNFSRQ3FGL J1640.6+3945NRAO 512?ïþ$0
 ?%"3[³©Ó?-¼þ÷_ÿ	?%"3[³©Ó?ïó]†T(²?`¦.{?YDóL¯ÛK?`¦.{?ïœÁ;kˆ\?‹O­Wà"]?ˆÏ±Ï%?‹O­Wà"]?ïþ€Ÿ€A?$9çlÂ?/7÷F×­Œ?$9çlÂ?ïùÆ\'Ÿw?D"]O-4?H捊 žª?D"]O-4?ïÙ2@ˆ±?uýxÀ?sfßû+C ?uýxÀ?ï¡ó"Ú¡?‰ö"'Œ!f?‡ƒÆ»¼?‰ö"'Œ!f?ïüYŠé[+?8¹c3¨}Ã?=3ª5úáÿ?8¹c3¨}ÃAGN4FGL J1640.9+1143¿ë÷/R¼@AJýTTÀ:%ïpeéÀ<?gÀÙyƒ@;‰³¢x@?Tú-X(?·(xD4b]¿DË*ؓ ü@'drñ9¿é¦Ž¼-ÿØWv¿$·¿èt­Q'Ñ¿ä0œJNì¿çâC5à?ª	CÜ´Ý~AGNbll3FGL J1640.9+1142TXS 1638+118?ïñ¹úžRw?mmUhÉ4j?\Œ
DérW?mmUhÉ4j?ïìh^–Á×?n"™á!Gj?c—¡@Ù·?n"™á!Gj?ï²N›2dÆ?€*Yéö?ƒlY,/ ?€*Yéö?ïáR˜~;š?Xr
.c2?n­gÀý5s?Xr
.c2?ïÁ¯)p3;?}¢YUé?(k]ãâE?}¢YUé?+¯ä½?'ÿ–ää?ˆÜu!Å@Ÿ?'ÿ–ää?ïeS¶?–J'º3&?œÿs\%í;?–J'º3&?ïJ丯g?"<Åð
3?–£hëÊë€?"<Åð
3AGN4FGL J1641.9-0621¿Æ¾Oj0~@9íÇïzÀ9'-åìXƒÀ;©pÑ#s£@
+¢F¨@68ù€Š?·EH´yĽ?ºþð¶`ú—@Wš»ØˆÃ@
ÉÂK"}ü?ïKøQÆ¿Õ}Þ€iG¿âÄßÎ1PÛ¿á߆®Š©¿êb…Ñe¸Á¿ïÿÿ" 5•AGNbll3FGL J1641.8-0619TXS 1639-062?ïñ­öYf?ZҖ¡}ÏË?\¤Á6\?ZҖ¡}ÏË?ïÐ(‡^?ƒç|ø^®?wþk²(ý<?ƒç|ø^®?ïw`3=çd?Š?´Öô×?'ù™úáŠ?Š?´Öô×?ïÍ¡Åg?s
?Eªf?ŒŒ—Ÿæ²?s
?Eªf?ïk—€î/§?ŽS&ÅF´?'Ù£9?ŽS&ÅF´?îü½Y"—@?¨Ôûøçæa? 4*kB×?¨Ôûøçæa?îZܒñƒ?žŠÊ¶×sî?ªR6Ò¦µÊ?žŠÊ¶×sî?îo†(2?"—
š¤
Ö?©žìzQ?"—
š¤
ÖAGN4FGL J1642.3-8108¿ïÿÿô¹È0À6+¢±pPÀ:ŸØvN:öÀ<$iϘ@«FjGœw@âWãì¤?À<'ùn@z¿¬\[p¿?ëXm_)]@ã%Íïâ|?ᄅSK¯¿ãI€2Wk¿íeK´3xÓ¿ä¡ãÀ¿ ;ƒ'¬¿ç·fÔJoAGNbllPKS 1633-810?ïûҏÀŽ?98Œî""?@µÀéýEò?98Œî""?ïôoÙVÈå?ZZ<gÁ¤?W Mӟ†7?ZZ<gÁ¤?ïØT×a•
?w/àŠ0P?sՔ0Hÿ?w/àŠ0P?ïþfà‰Ã
?ö8¤¶×?)'÷Eå¶?ö8¤¶×?ïìM£¡Û2?bŒÓ£¿'?c²\$k^¼?bŒÓ£¿'?ïÈa/gC(?–ˆ£B³Ûo?{Ïh-qða?–ˆ£B³Ûo?sË1u?‹H…Ës•Ö?žãäÎÜ?‹H…Ës•Ö?ïëú*À'?\'_Üxc?dÖ>.?\'_ÜxcAGN4FGL J1642.4+2211¿ï˜Fé@BÝE¶ÃvÀ;rŸ'*_OÀ<£fô*ߨ@!"…]ÓE@°"—©Õ?ÏWŠ€wË?¬"OÓ|ê6?äØ°?ù?G@ž×ÈSkb¿îj.Ýc?ïü_#¦ù¿ëk><{±Q¿Ìm«ÿøž7¿á#ʪ³Q¿Ò^³ŸTC¤AGNbll1RXS J164220.4+221132?ïü‹;‡ëq?2¿¶:ßÊN?;¦%=Ìô?2¿¶:ßÊN?ïâÁ‡¹>?Å×,"¥ù?m>xMÓú<?Å×,"¥ù?ïÖÐõÙê?sµÃvWå5?töuôÃ?sµÃvWå5?ï葇ZŒ?Ri{8wf?gnxšü´1?Ri{8wf?ïñYŠF&?^'ûCÆf÷?]ÙM^æ"ë?^'ûCÆf÷?ï=H›í?•Ö.Ðköp?WÓìg?•Ö.Ðköp?ï»ý܆ ?"wi6A?ˆí-í?"wi6A?ïYGlP5M?‰'/ ªÐ'?"×yhòi?‰'/ ªÐ'AGN4FGL J1642.9+3948?éا2MHø@Dz'öè)JÀ89m;l½˜À;v†eà/@åëÛóÛ@dŸ¼ÉJ?£<!Þ?¥9w'.?ÿM€k_Ê@;ÿ>¹ú¿Ä©$&%Ä¿àXÔ!Õ½·¿æoP»v­¿åø˞#—	¿æ:%6ñ.¿àpë$¦¨vAGNFSRQ3FGL J1642.9+39503C 345?ïþwL<ā?¸#ùËöV?(‹?eÁJ[?¸#ùËöV?ïóá86Â?\¦Ðv Q?X=‹÷?\¦Ðv Q?ïÐ|Ðò1œ?€ï¨í{Ü?wÁ—nÙíì?€ï¨í{Ü?ïûg4Ër?5è¢q֛P?Bc-6;?5è¢q֛P?ïû©Óâ8?: ""Ô |?AX³jº<?: ""Ô |?ïÕ¹i‡qé?wM–2R?u#K[3‡‹?wM–2R?ï̖àÆ?f킡pÙ?ˆ¾á'[?f킡pÙ?ïö,@?P·m£Ê/œ?S§€Šñû?P·m£Ê/œAGN4FGL J1643.0+3223¿í皈×Õi@DC,¥zxÀ:»£?4É5À<#e_Ö)@ð¢S&˜›@üÄÞÁÂ?¿ôPßÁq$¿¡¾ò!M¶?áÓÆÞ@•Æ5ƒðe?ïôŸhËÆ¿éŠÃ=O¿â…yA	Š˜¿Ý|þ®F¿í™z"¿ï÷Ê! áøAGNbllNVSS J164301+322104?ïË{êdÀÒ?v9چ¼¤¹?zB
Ñ¿¿?v9چ¼¤¹?ïæÐÂáÍ¡?j…%# ?i/=^ˍ?j…%# ?ï@]¢6e?'"¢Ýè?—ôK·{'M?'"¢Ýè?ïœ+›ÂÇ?pÑŒº‡?ˆþu#^"!?pÑŒº‡?3
ç?¢Õòú?§ԏ?¢Õòú?ï·ÂÁ}…´?‡~°©
}?'O¬ý*ä?‡~°©
}?ïG*€ ¯?"DÏÕ¯?—°%t"?"DÏÕ¯?j‹Ã?—Ù.Ñ8Æ?¯µ—È{\×?—Ù.Ñ8ÆAGN4FGL J1643.0-7714?ï
‰er`À3æ‰enï¢À:Ϻ×5À<*•Þ#6f@ì¾ÝöÀ¼@$@Q(ç?ìÛÀ°Š¿¥IÞ}â?äxdFÑv?ÿIkjÏ?Ý퍁Þ<¿Õgˆ$|61¿ìÍÛ?¬=`¿Ü³Š;WÄã¿Ð¿'zç&ë¿ïÿüoQÇsAGNbllPKS 1636-77?ïùÖ]ø·??CVë'wúL?H¦ˆ$D)?CVë'wúL?ïí Ëâö?nÃJMáG?bßî]XZ;?nÃJMáG?ïËêlQ¸?u(ÝÿÛ%?z
ðʇ?u(ÝÿÛ%?ïùQW¶uG?5†?Yb?Jº Õç5¤?5†?Yb?ïØL`8Ç?r8Z˜´­?sÙüµ¨†?r8Z˜´­?ï¸>d·3?—Ìþ#p˜P?ðfÏ&Í)?—Ìþ#p˜P?•á‰?Œ·ŒVŒ"þ?Ôšyýí¸?Œ·ŒVŒ"þ?ï´è-ë›?vòˆ¼S?'ÅôƒÜ=?vòˆ¼SAGN4FGL J1643.5-0646¿ÔTÈÔŔŸ@8xoš™tÀ:/<"댫À;ç–{(@ 1"­ú#È@
*áU?À­ŽÙw*.?*äâð?ÃÂ
V)ØA@ÊÑGZÝq¿»z£à…¸¿êßJþ«í¿å.iՆ¯²¿ßµ×<è=¿ä?z™¤¿ØÊ=fAGNbll3FGL J1643.6-0642NVSS J164328-064619?ïüræ7¾?Oà'L­k™?<hÌMÈ5?Oà'L­k™?ïãèÐ8'?y…6'?l/øèGö?y…6'?ïèûC؜å?v}'´™kt?g¼[+?v}'´™kt?ïüyRÑo?%Ðî0'?<5oE?%Ðî0'?ïûò|Mû?:^äX1?@6â¾wR?:^äX1?ïKØõ5\ê?¢€BÖP?–"á[0´?¢€BÖP?ïì5rls?o"õ‹,?c÷ʍ"!?o"õ‹,?ïôÞ¥gX?GvBÝ,‡?VäCf_)?GvBÝ,‡AGN4FGL J1643.7+3317¿‰¼BXB ß@DÔk&¿‡À;œÑ¹ôƒÀ<æݝÕh}@"Yp)]Ç[?ó1°|4.?ݜöZ婽?ïþY!Yl@ÒÞ^ň@%4ºÇ¼˜?ïý*BsÂð¿ï›iGÂ6q?à´®ÈÕÇG?ᇆqž©¿»f͔ré¿å×táSlAGNbcuRX J1643.5+3316?ï?èù(Jw?°Ø8£šN?˜à㍷?°Ø8£šN?ï¦ÄTO¯ã?—*·'µÁ?†Nê<?—*·'µÁ?7ûâ?šA^'}7Ü?§%'O×?šA^'}7Ü?ïÒ$¿@â?ŒTK-fDÌ?œe»bðyË?ŒTK-fDÌ?ïR»Ùà[ ?£8
9h!?•¨"¾Í"?£8
9h!?îÀ 0^?»$Yñ,?£ÿåý,?»$Yñ,?îõIµ£ø?—	Ø*c¿? «d¨cE|?—	Ø*c¿?íÜ09{G?¬Dæs?±~4'=Ë?¬DæsAGN4FGL J1644.2+4546¿ãÒ}은7@DkŠC»À;hEÏ)èÀ<ð1Cnê™@ ºÞ؁â?ýÒ¥Ú¼j?Ȃõ}Åþ|?–g—á*?Ñiè;")@aÒ­âQ?ïï=Û,áà¿ãÃނ׶¿×ñʳ!¿âo‰û–忽àÿ´«˜Ë¿è-Ë_\ªAGNbllB3 1642+458?ïýU;y[i?'`V^Ï9A?5V#2?'`V^Ï9A?ïóÇz÷^?[{Dr_hÒ?XqVÝsÄ?[{Dr_hÒ?ïìSÓß?jÉÜh?cá¬#P9n?jÉÜh?ïõÝÁ ¹?:,´ëÕK?TEÄ=…¿A?:,´ëÕK?ïùó…?AÜëÎÛ{?H1é¿·¬î?AÜëÎÛ{?ïÓ¬ä¾ÊÅ?wG{¦À?v)Ÿê±Y?wG{¦À?ïíï^i2?lh
{'C?b¡'QE×?lh
{'C?ïÜ*?fÓ?d
<Ë^¡ð?qêà\ÄJ¡?d
<Ë^¡ðAGN4FGL J1644.5-4602c?ï…ïç•6¿Éýw¤ý%À8…‹W"<À9ï–
óފ@"#ÆX¿_@Ãûå¿?Êu´¸,?ڄ]<œ›@<Ÿ¡ñVð?øtÊÒ̖¿ïûŸH/Cº?ïåRj0'¿â8Y­ñ?s¿é˜´—Ká¿ïÿý±q&´?ïÿŒýÿʦAGNbcu2MASS J16444975-4559026?Ôn°®iš?Õì3Ëø?åȧ¨óK3?Õì3Ëø?È<¨6`÷?ÃpGr§´²?éðÕò'Â?ÃpGr§´²?Òµ_7Èï?³/1׌›?æ¥Pdˆr?³/1׌›?ÑT†azç?¶™d'}?çpÕ¼ÏB?¶™d'}?­ó4äìZ?Œ‰çÂ=õ?î ̱Ò~?Œ‰çÂ=õ?"föʛEö? ¥é½&ò?ïdÈI¸ä@? ¥é½&ò?°¹õÉ_?J´c‡Tl?íýÈÁ‹ŒL?J´c‡Tl?sæê+'ô?kɄ›î!?ïØ2*Áìì?kɄ›î!!PSR4FGL J1644.8-2154c?îøí²J•z@.}¶™"¡À9ώ—"À;VqÐý³õ@ô¸ßÚñ~@§¸
è´?Ä~eá†BO?©©žŸgäÁ?èyØÔB@ÐUjÀ".?ïþ'ýž%ð¿ÛåB{¥"¿ä'Ö÷ÈùÙ¿æ Üš*¹¿ßr&s!á¿ë†hšMAGNbcu2FGL J1645.7-2148cPMN J1644-2156?ïûNÆÈ·û?Cäàüs?BÄä£f¢¥?Cäàüs?ïǯ¡‡"?ƒ‡Ô²`Æ-?|~¨GIz#?ƒ‡Ô²`Æ-?ïŠ_Zê˜v?†§ßí
æÖ?h)AêFŠ?†§ßí
æÖ?ï⦱bÁŸ?QTRÄqTC?mYNvÂÁg?QTRÄqTC?ïð¼Jjÿ ?coBÇ¿‹Š?^‡k@Ê?coBÇ¿‹Š?îá'o±?²ŸÐ"+7*?§îñԇñ?²ŸÐ"+7*?î;¿KŽ? §ŒÈç@?¯D
_Ä%? §ŒÈç@?ï
'™³+!?ôr&dÍó?ž[ÇâÍØ?ôr&dÍó0AGN4FGL J1644.9+2620¿ä©Mü.±'@C.}=BÀ:T¨ÎÀÃÀ<NŒÂÂ#@1:¥mbY@ѓpŠ¬—?»ÍÆFö´?´"»;)÷ ?ôØ/ž‹q@
öäñ0Ú=¿Ûdï"¸Ó¿æ}U–4Š¿ê"n§}‡ë¿èç2^wÿð?ïÿٟC&ÆAGNNLSY13FGL J1644.4+2632MG2 J164443+2618?ïü&$p?9Æ?ÅLE,?>ÏÎÕç=y?9Æ?ÅLE,?ïïS֍½?hXù¯eã?`¬)ËtÂÔ?hXù¯eã?ïÔ-´n16?re•·1?ué%Â-?re•·1?ïúºpÔ©e?3PÛpè~?E;µiÐ=?3PÛpè~?ïöԝ¦™‡?YhqH	¶?RVÄ°
Ad?YhqH	¶?ïÃìfΞ½?‡ˆ¼Ùbýé?~	Ì©.Á˜?‡ˆ¼Ùbýé?ïËôe0ô?}ˆ"N5¤q?z͒¤Ì?}ˆ"N5¤q?ïÚnjs?f{)¿0 ?rðHàîµ?f{)¿0 AGN4FGL J1645.6+6329?ïhýتÉ@Bü½º
RiÀ9á07Ö0#À<hœo6ï€@T—Äw#@
‰ÎÒa?´¯[ø¤A?ÆãÛÅ~@<œÆtÃ÷@T)`vP¿Ó‹¾úýÚ¿àö4êK¿æ,%!øxL¿ë´×Á¯b¿çj¯Áy1š¿ïà18‡0AGNfsrq3FGL J1645.9+6336TXS 1645+635?ïù
²ñŽ?Eaè6Z´=?KÉ3ð ¿?Eaè6Z´=?ïô¨;?i?_²8gHå?WÞ¯¸;ޏ?_²8gHå?ï£%©²Á^?ƒy@Tw/E?‡6•š.à€?ƒy@Tw/E?ïù V¦n®?2¾LSÓM{?K~¥÷ô·X?2¾LSÓM{?ïõ¤Ò‡Ì¾?TŽƒŠgcC?T¶Zðf"ï?TŽƒŠgcC?ïÔâgéž??xŸëæBN?uŽÌ؅?xŸëæBN?îì©-'¼€?–\µFC<?¡5m*gí?–\µFC<?ïކb|™P?^"ÃJˆ?p¼Î܀KÐ?^"ÃJˆAGN4FGL J1646.0-0942¿à÷´ûß	@6Lp¸Ï¿ÆÀ:¬~T–ZÀ<®Ò@!2ëÇ@¦¶~¡Ç?ÀÝYâÊe¿©—ÿ™jË?êᡥו~@":îéW¿´Îž31ZÁ¿ìÔ)þ+>¿Ïؓ)'ög¿çÀXëS '¿©à¡•ø‹¿åý
a½_GAGNbcu1RXS J164602.3-094113?ïèBͯ÷?t]€è^è?gí½5¹T?t]€è^è?ïÍhh?†gñR~'0?yKõKBõ?†gñR~'0?ﯦҴ?"áÝyD?":–J¢ð?"áÝyD?ïîtÓD=Ð?N=
@Ûp^?a‹,×?·?N=
@Ûp^?ï›CŸ´]7?‡¸³l&å?‰/7†E?‡¸³l&å?î¢[clШ?­V<;‰\Ï?¥ÚIÊêÅ?­V<;‰\Ï?ïl=y÷ׁ?ø
u÷>k?'xPÆ,yÐ?ø
u÷>k?ïpO¼^s1?ˆòpæÁ?'ö{Ñæ?ˆòpæÁAGN4FGL J1646.6+7422?ïçƒ'¿á@A$'žùTëÀ;^#QA;À<ñÄ>ˆÑË@ï·=ïNØ@=â@ÒX'?Îð颜Ž?Èùª¦\J¯?÷ôt{Òß6@˜5ÁWú?ï°û€>~Á?Ù=B äfœ¿åoïaLK2¿âhˆ•â¿ä²¥¤i×4¿áþ·á-VûAGNbcu7C 1647+7424?ïüü"A™[?3TȐ›Î?8fÆPYž?3TȐ›Î?ïóbœçò?YO+ãèÛ?Y;­rí?YO+ãèÛ?ïàÃ^[wl?sô=`%5?o<¡³¦Û€?sô=`%5?ïèFæ!?GtÑj»"?gã¸Õ&Á?GtÑj»"?ïýž®MÓ?0³&*ç]?3
«ÊÆ?0³&*ç]?ïÑ·pw¿Þ?vih?w$GǏ­$?vih?ï·\+`<<?"+ºÆB?'(õ!i¯	?"+ºÆB?ï©qr!õ7?pþyɖ˭?…££m3ÞJ?pþyɖ˭AGN4FGL J1646.7-1330?ޕpo~½ö@3õZž²OÀ:ΐTvyÚÀ<)VlGQ@"m@JGø?þ¼I	^N?ƂcÇûÁ¿—ú¹š?Ð$ñüÝ
Ý@/¦(s<?ïüÇ0«™v¿éó5ò*T¿ëOŸ_¬8?'3CaK¿âFîœ*m'?¯¾
þV˜ÏAGNbcu3FGL J1646.9-1332TXS 1644-133?íÄ{'rˆß?ΖrE†Œ?±Ü#kýŌ?ΖrE†Œ?ïÚꛮ‹ˆ?|€yñ¶K¹?rŠ²݄,?|€yñ¶K¹?ïQ®•Ì}?ž
p½«º?ŸõÊ0¶^?ž
p½«º?ïøÃw×?9Ð!Ôt#?O¤ñ†Öv?9Ð!Ôt#?ïó€ä«š?i	Uæ§Ät?Xþ7Lv;ù?i	Uæ§Ät?î¼´Ñ$í˜?°ÂŸWù°?¤4²ñü©?°ÂŸWù°?îÙÆünY?¡DÀƦ?¢c:x¶p?¡DÀƦ?ïܑrG‰ñ?e,•…Nà?q·FÙ{Wt?e,•…NàAGN4FGL J1647.0+6040¿ê‰+"½È´@CAÚßµÝÀ;s €©ÌÀ<Äæ©å@àfgh@±ì¹ÒE?ËD௭­¿vÓÿŠÓòË?¬1¦|g?æ@5=†Å¿ïÜD¿L±‰?ïRuÚ¿èsûÿwD¿Û+κã–=¿äèÏÍ2MZ¿ç‡Jw—AGNbcuNVSS J164641+603930?ïÿ%óë°Ï?"'Lêï?AƒKi¾z?"'Lêï?ïö/•!˜_?T&ýâšÇž?S Õ…Õ'Ù?T&ýâšÇž?ïíLN+Í?g€:+0?b³±ƒRRÜ?g€:+0?ïúÁììIa?-[çKvÓP?DøL%np?-[çKvÓP?ïþ)̵®V?)±íBw¨?-c21sæ?)±íBw¨?ïÜeJŸ?sxÕö€í?qÍqê~e˜?sxÕö€í?ïÖ Tx+?~"]KÔτ?tïÕ«7º£?~"]KÔτ?ïå¼Üj?^Øs`Zk?jCûT
"?^Øs`ZkAGN4FGL J1647.1+6149¿åG EDØ¢@Cvÿ:Þ"À;AºrW5qÀ<éegÊ@:¹•?úƒŠéÓmÑ?Ôª;þ2öL?ÔzJ´Y8€?ûϨ´¿Í@G¢ŠY
?ïý#I±$¿íÙÁY|¿Ëì쥿ÖÍ.œ=¹¿ëuäޑpU¿Ò|¾aÏþ°AGNbllRX J1647.3+6153?ïñF¡w?Só$‰$?]r½À ¼?Só$‰$?ïó VÇ?VÐé)3[ö?X¿R¶:J
?VÐé)3[ö?ïnØE%ùå?†¨ &-i¯?'$÷Ta‹s?†¨ &-i¯?ïѱéF«
?Xõ¦‰»Ü?w'|Fâ¼?Xõ¦‰»Ü?ïG?^óýÑÇo?aèpGŠàô?^óýÑÇo?ïÕ¬XISl?vâlñkÐ?u)Óà%½Ô?vâlñkÐ?ï.Û[—?'‹µk·R?š.D—ü¹ä?'‹µk·R?ï}.\'[?uZ'«Ðâ?‹à´aü1Z?uZ'«ÐâAGN4FGL J1647.4-6438¿ÁÅ,‹_€TÀ(íêî ¬À9€éNã'âÀ<fåè&Å@4$ÕwkF@
¿@óW?±.q,"?§(¹vÙ¦?õA¼bò@ˆWƒŸ‡D?ïñ?Ù}¿à"P&‰Å¿å"ÈL4‹ù¿ãJ=Á+®Ú¿éˆŽ^Òô.¿§™(¬AGNbcu3FGL J1647.1-6438PMN J1647-6437?ïü£À )è?1	…]]Ä?:áü*Ûm#?1	…]]Ä?ïð	ý¼B?vAØÁl>?_ì:º
²?vAØÁl>?ïê&tˆèò?_øŸ´öÍ=?eً²0Ug?_øŸ´öÍ=?ïø%ý¯\"?;¹xnV†K?Oh	›oG?;¹xnV†K?ïò®c€-?RH4Oÿxò?ZÞ£ Bv
?RH4Oÿxò?ïÂÞ)Ÿ_?—,¦¯µBu?~ëèl¿?—,¦¯µBu?ï´­ {yã?…¥®·DÕ?'Ô—îß÷@?…¥®·DÕ?ïçè­º0?ZT!lºÃ?hR9ƒ8j?ZT!lºÃAGN4FGL J1647.5+2911?îdÓð
G4@C='Ýãu†À:É@š$À<gzbœ­@Ë["l@{k{y"?½†ý )Uº¿¥2!BùWx?è:±âe»F@öü¢R{¿ÔÖß?–¿é£(Ž"ƒ¿àSþO%Ø¿çOÞk…µ¿Ò34	òÈ	¿â^"3N&AGNbllB2 1645+29?ïüäË#ÝÞ?0¦¿êŠ¦£?8Ù¦<#ΐ?0¦¿êŠ¦£?ïòYo™&=?ae§Ý¨µ?[M!Q¤"z?ae§Ý¨µ?ïî»?\é=uoƒ?aèùêÄYä?\é=uoƒ?ïúÄrÇY?,´3ž#ß?Dî4»ãÐ?,´3ž#ß?ïì­O®éã?^}0¤T?cR°Ü
k?^}0¤T?ïÆøe¾?…9S\ùt?|ƒÍ=)½ÿ?…9S\ùt?ïà:-A_?s@mí:è?oÅêàXÇ?s@mí:è?ïà+™g[?`¦Sïqäˆ?oÔfß\Z?`¦SïqäˆAGN4FGL J1647.5+4950?Ô^A{—ÈV@D	õ­–¦ À8ú'ûnjÀ<GùsôÄc@Ô)«|ñ@î¸D‹Ñ?¢²o~hß?Ÿ}ÀzNŒ?ôQ.ül͉@3L´äx»¿¸þö?·Ðç¿âíæÝð
¿¿æñਠñ¿äìö}Ë1í¿ã¼¡Ü^:H¿äÚ;JXêAGNbll3FGL J1647.4+4950SBS 1646+499?ïþË·ùÖñ?ƒèeÁ?#D} ­ÿq?ƒèeÁ?ïö^ؗJ#?W\^7´En?SBNýfº?W\^7´En?ïö`¬¾™?@.íð8?S>¦Œ!Þ?@.íð8?ïü‹#_*³?/WÑf§6`?;¦æ
rî?/WÑf§6`?ïþÉ×yùì?Ïÿþ•b?#b‰¬n°?Ïÿþ•b?ïÔÛ¼ N¡?xAz*Š?u'!ú×o9?xAz*Š?ïókä÷Þ@?aƒü~â"?Y(5¸M€¾?aƒü~â"?ïù£UÁ8Ö?AÃM*
â?Ir¨'ËW?AÃM*
âAGN4FGL J1648.0+2221¿å8ñ¬2Öõ@BD±ëÕÀ:!Øb,EÀ<MˆGa¾a@¾úWI'ñ@7~0‡‡?ÁžsˆØ›?Ë$ƒB@† Ä0F@b=Í@:?˨c`øh\¿ãR@>´q¿é†k>'aí¿ç<ÛR¡"¿ïÿô¬å¦¸?ïÌ®.|NAGNbcuMG2 J164800+2224?ïГd\‡&?s!‰ØPwˆ?w¶Mäú=?s!‰ØPwˆ?ïétJCŠ?ná<†:^?fê‹ò5•Ð?ná<†:^?ï˜q=¯ãÞ?€«$/,û?‰ã°"ˆ?€«$/,û?ïç3ÿ¤€?StÏ`Öÿ‰?hÌõúgÃ?StÏ`Öÿ‰?ïyzI"•ñ?'¡e-ßo?Ð¶ÈE×å?'¡e-ßo?ï•R¸)/?'KmõgP?Š«~ÀǨB?'KmõgP?¨)v¾?œâT&%Œ4?§$U€Ø0?œâT&%Œ4?ï8ý˜Øº¨?‡ Ä+ú•ï?˜àLèXFþ?‡ Ä+ú•ïAGN4FGL J1648.2+4232¿Ú`áÐÁ	@DË)^žÀ9¸xq*å‡À<wÜygË@öO+â1
@0‹¹F?±àÀõ~å?´
šGiv?ý œ˜Q›@ýuOÐ?ïÿÿ>¹ú¿àW¤ª²¿æg9ª€¿å9‡`1&¿è¾uñô¤'¿ïáãµFžJAGNbcu3FGL J1648.0+4230NVSS J164831+423322?ïü½]÷Š™?8½ÚQù÷½?:—õr¢?8½ÚQù÷½?ïó5,î±µ?b	ïwY™?Y•¦N—•n?b	ïwY™?ïÜꁓ"p?us3w}o?qŠ¿J$Ê?us3w}o?ïü"ÿ3¯ã?**Oí"·¡?;X|äK?**Oí"·¡?ïúý3
Þ?Lb^"iê¹?D3›ç¤ë?Lb^"iê¹?ïÔû×>ð?y@"Q²þÜ?u'Z""?y@"Q²þÜ?ï©Ñßþz;?…<‡½Äu?…‹ˆá?…<‡½Äu?ïùãaÊÜn?:n5sꪜ?Hrwþ³f_?:n5sꪜAGN4FGL J1649.4+5235?²ø,äôèž@Cĵ¢
ÜbÀ9*ÃÁ‹P+À<<ôE·š6@+Xäʑ@J¾A?¦?·>ßÓ?ª|·õ@EøÒåÂ@à?pXX¿Ü
²ûjo¿ßŸÀdµ¿âra ä½¿ÝN	îû̿䆃—¿¥¿åõ'ž}¯AGNbll3FGL J1649.4+523887GB 164812.2+524023?ïþ½]3þ?¯~÷«$?$*-\­¨i?¯~÷«$?ïömšÄ'?UÉ]‰ÏsZ?S$ÌX¬Á?UÉ]‰ÏsZ?ïõ®Ûu1/?bDµk{°?T¢H¢*Á°?bDµk{°?ïüÞ	àÿ_?(=Vˆ×H?9±G/<š?(=Vˆ×H?ïþ¤PµWÄ?éfÝ/c?%º÷°'&F?éfÝ/c?ï×NøØæ®?v»ž[06ƒ?tXƒ˜\?v»ž[06ƒ?ïô¿ë??g"ójN?V€)ÐòÂô?g"ójN?ïú´jfŒb?9æ`†Òõ?E.V3:Ú?9æ`†ÒõAGN4FGL J1649.6+0411¿ïõêØj@<åý2Æ&À:!$^"ÖÀ<	"&¸Ñ@J°7•Ãv@ürâu«~?ü}õ#X?ÆžÙtzü?þf"¿?E@Ý\"è¿ïÿÿ)@k*?ïÿúÁҝǿé¥Ñ¶@™M¿âO¬{­¿ïÿþó…õ?ïó˧nnAGNbcu3FGL J1650.0+0356PKS 1646+042?®]mf?²ìrŽZù?"vcw?²ìrŽZù?ïàZTšœ?xŽh@aÁ$?o¥«½‰ì?xŽh@aÁ$?îC¯ I¿š?œÝñé6Ç?«Å÷ôja?œÝñé6Ç?ïøw	·ó?:ì»ùta5?N#Û¸ThX?:ì»ùta5?ï¿ÇǬ?œ&Güé¬?€<'?œ&Güé¬?ïgRQ()?ž{j\ÿ°0?"µÒgôä?ž{j\ÿ°0?íãÖü?¥=oD'ý%?·XáQ?íê?¥=oD'ý%?ïÐ¥\E{4?oÄT¾I?w­QèñÆ?oÄT¾IAGN4FGL J1650.3-5045¿ïÿÕfŠ‰ÂÀÈ þÀ7ã',"³À;ýº@¾
/=…G@žÞ|øy#?¡ƒfÁþB?§bܙË@ô6%UúÞ@aŽQ?ïûûß	s¿äT^¦ÿ^¿åŒ|Dôü—¿ä÷'ê)Õ¿ä˜æ€Òù7¿å÷>àæ_EAGNbll3FGL J1650.2-5044PMN J1650-5044?ïþÛQ?$>ù9Öà?.BN/	do?$>ù9Öà?ïç³Nw˜?x`ã8¬ÁU?hLì'ëÿ³?x`ã8¬ÁU?±ç)?‹°•«ð¬?‰^Ӑ"sÍ?‹°•«ð¬?ïþ¦¬°*]?\QOQ
?%•6BΑ?\QOQ
?ïûßö[w±?<ä!%2JE?@€&ɽ?<ä!%2JE?ïDav×<?§Ön¶;ò½?—~"Ñ%‹?§Ön¶;ò½?ïd-dù:$?'šÌ­>ÓU?"zSioÁj?'šÌ­>ÓU?ïý¦i¿>ø?,À³«DÄä?2̱'{å?,À³«DÄäAGN4FGL J1650.7+0831?·ùtRe½@>¥¸fä:¨À9²rùòŸÅÀ<<(¥:¸@Ñ
NG6@Øró<£?¼¸«­˜T?Ãy§¶½ÁÂ@°~ZxòZ@SaÅ¿ÀŽ|2iµ¿æï<™
' ¿äE`ýpه¿ê®HÌ]ç¿ì1  œWº¿ïÿÇ*Ì\eAGNfsrq3FGL J1650.8+0830MG1 J165034+0824?ïôÜ
'dõ?]…Š	?VGê|Äwm?]…Š	?ïãbñ€¥?vÈ¢2$Ùi?lå.¹?vÈ¢2$Ùi?ïœ;rFïS?ƒåZ°û3?ˆñ#|›@?ƒåZ°û3?ï×D=èï?\nÌ)¤j3?t]±€§ðs?\nÌ)¤j3?VæŸ9?‡Ü¸j,S?ˆY*8™Á¶?‡Ü¸j,S?ïbR‰Ð¬?›Ü(64Wf?"µ¿«VNy?›Ü(64Wf?î¿ÖB¨'Q?œODê2?¤›ÖSÁñ?œODê2?ï;V3Ø
Œ?'©†f€üa?˜•9ˆmêm?'©†f€üaAGN4FGL J1650.9+0429¿ë€š«â@<À%á;ÛÀ;Zœ-ȐÀ<r¹¸óÑô@!a‰óß5Z?ü«+­,ôU?ЮúS?µJ;"ý¾?æ5™e—4@Ð}
œË¨?ïÝÅB"пîJn×N0¿Ö4œŸˆpý¿âBá[Ð
o¿"*å(Z´y¿ç"Ғßk5AGNbcu1RXS J165053.5+043009?ïüRõ¬{/?3¥§kni?=hRÍ èÞ?3¥§kni?ïâw!°»?|vPƒÃöè?mˆÞ.H»¤?|vPƒÃöè?ïݐ©j-?t»3Ç& ?q7ñ¨A4?t»3Ç& ?ïò•¹/
?D$®KRÀ	?ZԌf¯§B?D$®KRÀ	?ïúwai?GZ?‰‰õ?Gò"yÏ2|?GZ?‰‰õ?ïJ}ùÄÁT?¢'wDXj?–°@̏?m?¢'wDXj?ïÕåǁs?}ÞKàE(?u
.â«?}ÞKàE(?ïÀš©'ðÏ?t‡W'+Þ?²«"ÄȌ?t‡W'+ÞAGN4FGL J1651.6+7219¿êl¾vÀ3@AZ*o?RüÀ:u¤åýö;À<¨ÃФÉ@ €ç®z|H?ýùiÈñuú?µÕáswñÔ?sñ‡l?Á«Ü<Vr}@bô6H;ƒ?ïӟ县Õ@Q~Í»_¿â#îâvWJ¿á{ý§`+º¿Ø"ÿ^ow¿¼âÊ [PoAGNbll3FGL J1651.6+7219RX J1651.6+7218?ïý *hš"?"Ímk}?2þ­…{BC?"Ímk}?ï÷"üb?UuªJB£¦?QÛêûûš?UuªJB£¦?ïöÕéoß{?TïŒ=Ž?RT,ÂË«?TïŒ=Ž?ïõ¥ÇáfÉ?<‰
:ˆz?T´oÚ=®£?<‰
:ˆz?ïúÙÓ™´?;cÙ¤(?D˜²µLI·?;cÙ¤(?ïÛ¬pƒB7?sàs&Ð?r)Çʽ|š?sàs&Ð?ïñÏãO­?pG"7³·.?\`9(#5h?pG"7³·.?ïèøԉüæ?S†§Öž‰Ð?g+GHjZ?S†§Öž‰ÐAGN4FGL J1652.7+4024¿X|Ïq]^'@Cb¯È°À:™":ÚÇaÀ<q.~˜ŒS@ Úàl'Ο?ýC$\֚¬?ÆuÌ4÷X'?´o"3,'?ñÙ«Ø`@ªÅ
¶'N?ê&둳ò
¿ãþÀZN¿Ï¥_ö_Ã4¿àXŠp0ꄿÜ®½î¸¿Þ˜âºtÛAGNbllRX J1652.7+4023?ïþ¼4½æš?ˆÝœã/?$<´OÄVÞ?ˆÝœã/?ïòo—ý?`&‡DלF?[!çUïÁ?`&‡DלF?ïùyÙ_Ø-?TcÆÑó–¨?Jš9'm?TcÆÑó–¨?ïë@æؚ>?F-R@Qˆ³?d¿ñËÚ>?F-R@Qˆ³?ïþ#ºwé#?#PÚt0E?-ÄW'¼?¬?#PÚt0E?ïÍ9b]~r?|/=~xb?ycNáû'?|/=~xb?ïû5×cÙ?Pâ0ë¿?C(£ €?Pâ0ë¿?ïÇÇ
QMâ?fjȥꘌ?|zÁ[Q?fjȥꘌAGN4FGL J1653.8+3945?ç)Nû22@CmZ¯xþïÀ6Ę¹ŸÉ_À:½¿_ü¿Ú@7o¡Îqh?û‰¨U?†?‰i<¯ˆÄ4?"hKeP‰'@
gý?[`@0''àCÍ?Ú+Ú佄Z¿ÕÇ+£ù[¿Ü2Ÿæ¿g¿ÖPñ_(Y¿Þ"ÊÕ{Ç÷¿ÏU)¶³AGNBLL3FGL J1653.9+3945Mkn 501?ïú¢i]"?Hi×ÀŒ?Ev[LnÚ¼?Hi×ÀŒ?ïó9I3?^—Fwm}½?Ym.¶/ª?^—Fwm}½?ï|vÅ6ß?ûˆ›Y5?1#éˆ'?ûˆ›Y5?ïþñݨg=?,ÆlF;4? â#}'?,ÆlF;4?ïòø²·
?Z‰×ó?Zœ&Æü?Z‰×ó?ïÖL:ɳ?x4¸d'q?tÙâ|éâì?x4¸d'q?﹑`‡v¤?‰EßxÅs?›§ëàÆü?‰EßxÅs?ïÿhã:ÄÄ?ËFŸÎ"?㛉Öæ?ËFŸÎ"AGN4FGL J1654.0-3509¿ïêÛÉ@˜W€ðUhÀ9ª6CˆìÀ;'ã}zV@)Bnº@¾aÏþ°?½n'¥áP'?ªŸÀÊØM?ïºÿ?8$@Øד¥8ß?ïÿ®©Ì¿äÿà iA¿ãpWìPÓ¿à¬ÿ'¿çõò•´1Ë¿Ô©ãßVAGNbcuNVSS J165404-351301?ïøÒÑ7"j?H7¸Job?L´¼º›K?H7¸Job?ïÉâ'ÛV?"u¢Ÿ¡ÎK?{q¿BA	?"u¢Ÿ¡ÎK?ïÛ3a<—?r|þ'=©ª?r|f\p8`?r|þ'=©ª?ïØY?âC,?[r߄Ù?sÓ`#|?[r߄Ù?ï犼˜2x?dÇñ¦|?huC€Š¸V?dÇñ¦|?îy«?´zK//@Ö?¨gM'ÞS?´zK//@Ö?ïLÀ¥b?'*/€Ñ@?–gþ¦j‹°?'*/€Ñ@?ïUA"¹¥?‡§HEè7?œWҐ5a?‡§HEè7AGN4FGL J1656.0+2047¿îü œz@A$äâmHÀ:!ãû½{ À<RNöÞ@-â´?¸'@ŋûKeY?Á'ï@À£?ɹÀ€Ž/Ù@ꇅšß@8q¼Æ¿äDFŽ¾¿á[©t0¿æ<ït—'¿çlãË¿ìK`†R"ø¿ïø¸®1×AGNbcu3FGL J1656.0+2044MG2 J165546+2043?ïÒQ;åg?pƒ$@0ܔ?v×bÔ?pƒ$@0ܔ?ïè4HÿD¼?umwGQg?g˶Á'tÅ?umwGQg?ï§ÝÚï­Ö?~ï²¹Pó%?†‰6V—?~ï²¹Pó%?ïêXüùîÍ?M""BŠ‹L?e§F©Û"?M""BŠ‹L?½[Pð?ŠFw¡ã?Š³z˜?ŠFw¡ã?(Ü?—ā/Þ?‹™ÜG"
?—ā/Þ?îC0Ðÿ?ŸBœØth
?«Ì÷ð4?ŸBœØth
?ƾë¹?v`eb[È?ŠNB†¡ë?v`eb[ÈAGN4FGL J1656.3-3301?Õ@ù	k¹Œ@hH'ÓÀ8ç
ÜÒÔNÀ;)yÙ	ò@ÆGåœÒ^@Ršäó4@?º­j˜?Ót¯'@T+
oÆ@"4A{†¿Ïñ@õh¢¿ä^2.o¿ê¹Ë"}®W¿éY<a°@¿í-F¿×ñÄ¿ïÿηˆ—êAGNfsrq3FGL J1656.2-33032MASS J16561677-3302127?îSîz¶C?´]'7)ÊÅ?ªÏÄ7Å?´]'7)ÊÅ?ﲏOFlÔ?Ê¬²­?ƒ\,"^(ô?Ê¬²­?êãW³ùŸÇ?ªÀ™}^o?Är¡0€ã?ªÀ™}^o?ïÞpZ¨d…?[ÔîDáh?pÇÒÂ{)]?[ÔîDáh?ïC I>%?§-lN ¹"?—‹öÇ0Ñe?§-lN ¹"?í-Mç6ö?½T/iÄ?¶•ÅfzS?½T/iÄ?Ꜩ¨]à9?­ÒÆĜ"?ō]^ˆ?­ÒÆĜ"?íÛß²¶(Ï?£ˆ¢ÅJ?±!j¼­?£ˆ¢ÅJAGN4FGL J1656.9-2010?ÞRoêÎb@,5inX£À9j›‰]â3À;âxˆ§ÙÎ@ z—éJ?ýT¼ÕÞÄF?´³£(2ú?¸öª蟑@í^µ˜@J4Sï–P?‡µöØ %á?ïîÛJ>´¿á2"¢¶‡¿ÝœŠ$[©õ¿ÚºØƒA&¿àäõ¦n"AGNbll3FGL J1656.8-2010NVSS J165655-201056?ïü4'"±'?IøÃåOÅg?>^Áø¶+Ò?IøÃåOÅg?ïNÌ€Ÿ?¥º[Ýb?–.u%v%?¥º[Ýb?ïÉ­¼¢nf?})]˜À?{)!œ:éJ?})]˜À?ïwÃ"©ù
?tîÚóêë?'›©	Y?tîÚóêë?ïô%E¬)?ZùdR3'O?WµtGxÛ ?ZùdR3'O?ëc_-b
ç?Å¥$ÞŸ?ÂrƒJwÈd?Å¥$ÞŸ?ï®%r³Ú@?‡³ý»/«?"v£FªØ?‡³ý»/«?íõ`•Ó!·?›Ã	…ýÚ?°TûO¯$L?›Ã	…ýÚAGN4FGL J1657.0+6010¿¤7êeڒm@B´iaÃiwÀ:~oPóÇÀ<¥ôõ
¸@™'Ǿ,@cg]Ý*é?¼¥nS"Œ?¢ôšàÛ;i?äXy¾²Ø°@
	ú
å¿á†*Qb¿âO¾Ÿ !¿æïŽÎd|¿â°ô>«·S¿é¬¶ApØ¿ïð‰À]¨¨AGNfsrq3FGL J1656.9+6008RGB J1656+602?ïýF
ë_?'MÎި?5Ï©J—RÊ?'MÎި?ïöÑü·v?Sû›Iñ"?Rü[±ZÄ/?Sû›Iñ"?ïîÛxóB?\tƒg'Šÿ?a$†ÛC"?\tƒg'Šÿ?ï÷f%ÎÆ¢?:,…¡©?Q3´ëã ?:,…¡©?ïøûÃ¥?D~ŽÖÚÞ?LóÃBYX?D~ŽÖÚÞ?ïÙ	¥´ô®?xÙ«¢Æ—?s{-
¸µP?xÙ«¢Æ—?ïì¤p¸#ó?j*öm€?c[ ¼ê?j*öm€?ïßjÀÿŽ?]|QÞÆÓ?pJŸ«}/?]|QÞÆÓAGN4FGL J1657.7-6120¿¼š—¬•°èÀ&¶"áÉ´À:ˆ™'6À;èZ§ìB´@>tà&ƾ@Nõ>M?ƛoG5ž?rŽÛ"T¥
?¢bÕã ÷@`Ü&$?Þ©'`ìÿȿꯍâ+XÉ¿çù¥=;ʱ¿Ù^–C"êf¿ë2ˆä?°¿€m»qAAGNbcuPMN J1657-6121?ïðY¬6%?a`¯Müf?_L¨EH$'?a`¯Müf?ïïö«v"?hI:¤Ë5?`	T¨#ü.?hI:¤Ë5?ïÃӇ"¡Ã?{E	ŒÞX?~<$ñîo?{E	ŒÞX?ïù'c€X?2<Ï,/¾?IõË(ƒx ?2<Ï,/¾?ï䯆ã*ÿ?f¥Js1ù?kPy^̀%?f¥Js1ù?ïºܖ:â?˜|¹äý@?Èäh%?˜|¹äý@?ï{€‰¨4è?'.øì'?îÐ Ìü?'.øì'?ïÔJ;°?eËમv—?u÷tÒ£#?eËમv—AGN4FGL J1657.7+4808?àI¨Sîh@C=½øôsÀ8'BhZ\mÀ;ü¯0ړ_@mE÷0"³@xÅÿS1Ö?¡"ßíª­?¼"N^‡Êº@	0¾
í)@q܂!ƒ?ßê
 AÿT¿âɱgì¿åù»þHoÛ¿ç	õíW†Ð¿è"9-H8¿ë3Ÿ¿£n…AGNfsrq3FGL J1657.7+48074C +48.41?ïûüÈ(?CÈÁ8aò?CÄ
Œã¯9?CÈÁ8aò?ïå¨ýÔpt?t½û8ß?jWTÊÛÒ?t½û8ß?ïÚ®=Pԕ?yê¿\¬Ï?r¨áG•˜?yê¿\¬Ï?ï¢ö?M V‡ë¿»?alMÃCÂf?M V‡ë¿»?ïüÞ•|e?4îé	Ž?9Õ5²äS?4îé	Ž?️¬ÁûŸ?†6ö°®?Ü˹†Z?†6ö°®?ïáìÀCb¼?x>ÙºË?n?›¡º?x>ÙºË?ï¬ôÔÅG?rïLsáý?"Âؘ?rïLsáýAGN4FGL J1658.4+6150¿ìó]ýƒ›@Buø"»ì«À;
ºª‹YeÀ<ÖFô@>#âÞ1#@ _¼(9Û?Çõ°[R;?¬`j_*™?á6É™"{@([DŸAN?ïaÜ>ñ§¿ç_d¥Ï2¿áȼœÓཿÔ|y"UÀQ¿ëþáòο¿ïì=ÆþAGNbll3FGL J1658.3+6149NVSS J165808+615001?ïïÞ²}k;?VàVþÒ ý?`!MtÖU]?VàVþÒ ý?ïòÔþkø™?X£f›Æ<¶?ZVQž-?X£f›Æ<¶?ïÂPpl	û?ylÒô~¡?~×Çәêª?ylÒô~¡?ïƖéÕµî?`é=sŽz$?|´‹*rœ¹?`é=sŽz$?ïÙué!}d?p0×ÞWä?sE]cUã?p0×ÞWä?ï×ÛSxM?rnO&Dì?tVcuÛx?rnO&Dì?ï¼1Wž:?…DbúXó¢?€óª1™a…?…DbúXó¢?ï9ül÷,?€ãµì"k?˜ÀryÙ°—?€ãµì"kAGN4FGL J1659.0+2627¿îct-K¡@AªÅO±À:±räùê<À<Q
¯ëëv@7;Îßw@'¤/?ÎÖç,õW?Ò(ŠBŽšã?úð"!'÷¿@ßëR?è0ál—¿èt9rèU¿èB¤À>I¿ìCŒFÊ¿¬¿æÑü·v#s?¹`4žWµAGNfsrq3FGL J1659.4+26314C +26.51?ïû¡}#þ?B(€zUZ÷?C•zûƒœ?B(€zUZ÷?ïäǛŠ‹?|ÆMPó'ø?kà8.ۍÂ?|ÆMPó'ø?ï–AIî­ë?ƒãYˆåð?Šo­z±n?ƒãYˆåð?ïÎôÍÐ`‰?\Ô,>®°½?x…™
€ç´?\Ô,>®°½?ïù`†ž.?PíáÍK3?J¡Á>›?PíáÍK3?ïeԛ«Ë(?šPq6?"ElˆÎÍ?šPq6?î«aóeþ?ŸúÇáõ`¼?¥IàÉ®à(?ŸúÇáõ`¼?îÝ$?™	ZH€4?®xüº_¿?™	ZH€4AGN4FGL J1659.7-3131?ís/¨¢@Òø_øŽÀ9@Bæ.žÀ;'ëƒq9(@5ïù>@ðú#G,å?³ÊL¿Ì3J?µö<Ý«í.@=Õ%`â™@¤÷;
m?ë\ûÿr©¿ãt›Gï'ڿ收:º2¿Þo•¤—y"¿åeüH»Zµ¿ëÓŒÚnvAGNbcu3FGL J1659.7-3132NVSS J165949-313047?ïþÉC^?"÷ØZ`>`?.³oùŒ=?"÷ØZ`>`?ïϗx4͛?'ü_«
«?x4Cú6ڋ?'ü_«
«?ïí|~Åq¨?böZiGâ+?bƒ;î/€?böZiGâ+?ïç"ƒ¢Y?QÎ'}õ‹?hól¦øÎó?QÎ'}õ‹?ïüi'â?8x©W¯ª?<³ð¿×õz?8x©W¯ª?îzÒõìçÜ?´4ßßæ?¨RС1'H?´4ßßæ?ïÐÇè®Ìÿ?w ͚?wœŽ|x­?w ͚?ïŽËŸG¥Ó?yf}M3Àœ?ŒM?D—?yf}M3ÀœAGN4FGL J1700.0+6830?âC!3Æï@Aš¸¾øγÀ89FÍCëÀ;ׅJW<'@Â]ûu­@:>xá"?›Zm^Ó!?ºŽTììQø@ÙùŸ"®ž@TÖ}АQ¿Ú Ä܏û¿á1ìv¶?ÿåÚò)}¨¿æóe½Éû¿êÎ[–x¿é\°9ïAGNfsrq3FGL J1700.1+6829TXS 1700+685?ïô
F˧š?ThOŒ?Wår,kã?ThOŒ?ï릚ð?qÔÝð\œ?dYeE'×½?qÔÝð\œ?ïÊ%ÿ7Õ?€¾¹hˆ×?zíP2I‹?€¾¹hˆ×?ïøçØkçZ?>ðK"lWÄ?L`~íR?>ðK"lWÄ?ïÙß_Õ^?o¤.l%ÍW?sPx÷?o¤.l%ÍW?ï¼ùgæÂ?ˆAç+ä<?€Á¦'Å_|?ˆAç+ä<?ïÂQ5Ë?…WeðßKŒ?~×|ݯö¹?…WeðßKŒ?ïÛ®5¡¼B?fß9œeõ%?r(åN[?fß9œeõ%AGN4FGL J1701.0+6613¿ë,©ÿ˜Q@AÙR*o?SÀ9ì¸c­OÀ<y7ýO1@ë‡('çP@ÑBªŸ{?µ£*€ËÜ&?¨o¡"2
?í'Q;[÷@J¨¡tYn?·ä£Ù
¢Ö¿æêµ`I–Í¿è"œFó˜¿êƒCÿEÆ¿êí«i¥¶¿ïþ;âÐAGNbcu7C 1700+6616?ïýŸ´L¨?&%'J5÷‹?3\Já&?&%'J5÷‹?ïõ¾Ñ È?U/7/I?T']ºÀ)?U/7/I?ïçm¸{?eøJñj6è?h'r‰æme?eøJñj6è?ïëÅáK4?S£Ýl"?d:·‹ª?S£Ýl"?ïý¬‡C;û?0JåkåZ?2›Æè3ò?0JåkåZ?ïÜÀHã|?qì%	©;î?qóŸåÝÐ?qì%	©;î?ïí'6Ú?l¼Pk8ñ?bï}èÂXv?l¼Pk8ñ?ï¦ئÂ?uÃÉjL?†z‰È'	ð?uÃÉjLAGN4FGL J1701.3+3956?؀vœXTš@B¹Æ\pC_À:1!
;ÃÀ<Žgú»¡@ø˜¾ñî@2<ã¶^?ÆMO~˜a`?ʇò<ÈÞ+@£¼ÅîŒ:@GhÓ©	ú¿êZ…¢kÐ3¿Á‰¥…¶
¿áúâ‰Ít¿å–¸w«¿è×ãD8>¿ïú":½k0AGNbllB3 1659+399?ïåK'÷?j33Š!P»?j´Ù*ôr?j33Š!P»?ïè,=
´?j|Œ‹?gÓoûNä?j|Œ‹?﯎_ÌÛ?}¾=?_7?"h	ŒmM?}¾=?_7?ï¹àœ‡?b•ïBÓò(?‡ØüÛÞ8?b•ïBÓò(?ï91aÌÎ¥?šW±÷ò0?˜ÙÓÁ>Á_?šW±÷ò0?ï¸.p3wY?'BŠ	Gî&?ôcøù¡?'BŠ	Gî&?톷%Šlð?¨Š.;®€&?³ÊFÔŒ?¨Š.;®€&?î¯íËlqæ?ŽÖbý??¥#JÈ¥?ŽÖbý?AGN4FGL J1701.7-5621?ï|
þ¬À!Œû¼¾bÀ:f/Ш# À;—Œ™¦@4›Jž´·@ >ê šª?È Br–K? "…`Q¤b?ܬ®^͕Ë@Zª=€¿?è›×âTžh?ïÙ_æÌR¿éùJn¹?¿è¸æ0K!g¿Î°Ý˜wÄ¿çë$ p¸ÐAGNbcuMRC 1657-562?ïõáa7-?k/aNDø«?T==ý)t?k/aNDø«?ïÓ]æȳ?¯û&B²?vQv›
?¯û&B²?ï‰2"ú?†}ö	ñ?³zåP0­?†}ö	ñ?ïí©~òñ?Pß
/Òx?bV
~G?Pß
/Òx?ÛߗÞ?'þéˆ[ ?öëüŠ?'þéˆ[ ?ï$Foâ!?°y$#ãÄg?›m÷+$ƒÞ?°y$#ãÄg?îi¿õz?žÅTdY'"?©d«W¤Z?žÅTdY'"?ïI­|¿2?ÝÎh3?–ÊPmA&/?ÝÎh3AGN4FGL J1702.2+2642¿åD
ŠúfÛ@A\‹ÁiÂ;À:"E>ÎqèÀ<ƒ:"ÀÅ@%|nWÌ@®M]€ä—?Àóîº2kb?¬±<Úý?íS?ˆÖÿ@	d\1"1}¿ïû>¤€?ïÿbì^bŒ¿ãrí]f¤¿áÌ@µÒµ¿ãˆpîèV¿ãÇ(žáŒAGNbllMG2 J170210+2643?ïþ7¼À÷=?!¯HA20q?,"4¿A?!¯HA20q?ïï+"á×?fZȱˆÆ\?`ÔkË)–?fZȱˆÆ\?ïïéäNq?_3ZAâDû?`Ým>?_3ZAâDû?ïó3!{¶ì?Ah'³&Ö\?Y™¼Ù×x«?Ah'³&Ö\?ïü:ù"*?7J•úÇ·Õ?>/—½@?7J•úÇ·Õ?ïÂð½Âô?'œ'*†?~‡¡0|­?'œ'*†?ïðxhì?h€îjgæ?_÷ÝíØG?h€îjgæ?ïÓçєT?h)3µ¤*?vqŠ×=û?h)3µ¤*AGN4FGL J1702.6+3114¿ïü—kÓ@Aߓ‰µ À:R2#h»À<vòS4Z@ P‡[SÇ?üoøØ?¾Þsþªjw?³%ÏG{j?öh†>Þ@\'t/'?ïÿþBe«+¿ã¢UË
¯ì¿ÝþÄ+=›l¿Í¯u£ñp¿ÝÒõ:ªú¿âÁ<£AGNbll3FGL J1702.6+3116RX J1702.6+3115?ïüc`L›å?2z¹ðJzK?<äüÐÑrï?2z¹ðJzK?ïíã;ŠUë?díQËNpo?bĆ(4ê?díQËNpo?ïê®@?¿?rHŒG^ÖÖ?eQàÃßÉ@?rHŒG^ÖÖ?ïٓv·8Þ?Rκ׏šþ?s6D Dé?Rκ׏šþ?ïú.7~z?BÌaø<&²?GG!uÚ?BÌaø<&²?ïÈڀ·?¢ÚLÅ5?{þ Y¼á?¢ÚLÅ5?ïëÕ²é:°?oE'®Ž¿?d*MƏ ?oE'®Ž¿?ï"õ[q?qãiÉSºÍ?ŠÂ©0±ç?qãiÉSºÍAGN4FGL J1703.6-6213?Ǥnß±«ßÀ(â­ÄÉÉÀ8=֌i/oÀ;aª‡'§@G–¡—"Ý@áª$+Xs?¢þ\緊?ÃXeœ¼ä¢@Ê&½+.@Â*f…ðð?ïÿ«çy÷=¿áˆ¶‡¿åñ°F"HϿ婼'ì&.¿ë51ÛD^Õ¿ïÿø="ßEAGNfsrq3FGL J1703.6-6211MRC 1659-621?ïҚEÕ½?†ÑÍGM?v²Ý@Å
'?†ÑÍGM?ï¦Eró4?"sd3'Ï®?†yn•"Ã?"sd3'Ï®?ím´U?¦!"æŒ?´"'\
-[?¦!"æŒ?ïӝa'Ún?iԏQRÁ6?v1O@¢Œþ?iԏQRÁ6?ï2!9´?›D7æ–åo?™»ÜøY'˜?›D7æ–åo?îdp«I£?·œ­o@R÷?©¸þÿâ×?·œ­o@R÷?ëӝӚ?¬Ü¤8â}A?À³ˆ³å˜?¬Ü¤8â}A?î\Ý[îÆÐ?˜&çßó|?ª2*Aïyû?˜&çßó|AGN4FGL J1704.1+7647¿á_ËWµQ9@@1éÍ³}À9@UÁF‡À<M¼¢³Ï@¬ÙIÝė@S°ÄXŠ?§ŒàŸ©?‡–!jŠ?Üî~Î<9@­ÿ±%§Y¿ÔȨZ§–\¿ä_ÕÑXM¿èO/]e¶¾¿ã_lÂK¥¿éï81Ÿµ=¿ïW–Š •AGNbcu3FGL J1704.0+7646NVSS J170357+764611?ïô$»²Yj?g¥˜ºÓN?W¶ˆÜÌI?g¥˜ºÓN?ï÷"%ˆÈ?UB)ñm!‹?P×µu  *?UB)ñm!‹?ïÚIþYj]?{~4í"?rÛéHQR?{~4í"?ïÿ§$>9?J|–º?6â>ûZÔ?J|–º?ïýÞÚôá?5Q|aC†3?7ñ*,')?5Q|aC†3?ïÜ@BîŤ?sk9€fÜ?qßރͺ<?sk9€fÜ?ïÚnH]ý?|0¾©;€?rÈÛù?|0¾©;€?ïÿšÌ8l?y]
á$Æ?	LçËÍ5?y]
á$ÆAGN4FGL J1704.2+1234?ßò£ý
@=f°¦üX¬À:UÎyu6äÀ<E¢Ä»†S@'ê0µÕd@1wðÚÉ?Â#•ÜJÄ?µ(õÂå?ñK
¥uoï@
jŸHZ6Ø?îÔÎÞõÄ=¿êè±d'z¿Ö{%¥«ö"¿ä¤5~ç煿Ý@ˆ[XÁ7¿ïÿï0l¯AGNbll3FGL J1704.1+1234NVSS J170409+123421?ïû®#`ϛ?9‹ÇZº?AGs6™?9‹ÇZº?ïè¤ê¹$'?qŸ›b-Þì?g[âþi?qŸ›b-Þì?ïà=ÿ!^?u%~%]$?oÂñD6ùÚ?u%~%]$?ïó=a+áR?=.Ú¢É7?Y…="lÅ?=.Ú¢É7?ï÷/M£Ä?N…¸¿p?Q¡ï"s'Q?N…¸¿p?ïƒÌî?ž°ö-3?;Lø¥D}?ž°ö-3?ïÚj	3/'?{÷ë¢?rÊû\jç?{÷ë¢?ïÛ4à÷?\ŸmÍD¸2?re…ÕP¯?\ŸmÍD¸2AGN4FGL J1704.5-0527¿æó°å¡Á@4ʂƒÓ^·À9Nµ×½Á—À;ΛâI5Ô@ =(Ɲ³°@Ga)Ä?®tÉUží쿕æ…ZZn?éά€§f@ý³¶P^'?Øø¾RW¿ã‹rX¿äÍhø¿Ûr£áq¿à×{ýQyð¿Í;;~AGNbll3FGL J1704.4-0528NVSS J170433-052839?ïýHQõ¸v?(]µ›5,?5½r
V¼?(]µ›5,?ïÚ}És?×?yÐãësí=?rÁ*3Hm?yÐãësí=?ïîzښ?dâùg"Î?a…÷U€rÔ?dâùg"Î?ïëúø.Ot?Mú#ƒNè?d×/ìH?Mú#ƒNè?ïøaàR?GAÌ(§Í?O–{á˜2Ž?GAÌ(§Í?ï õp&{?©}æ~²_$?›áRX?©}æ~²_$?ïçËå,{D?upм<O?h4¤Êì?upм<O?ïÄʔ…ªò?iPù(µªÁ?}šµÆƒ ?iPù(µªÁAGN4FGL J1705.0+7134¿é[ÖQI¸u@@úˆ?Õ%À;%J<d4À<ÍB=Jä@úCºÚ1@‹Ó"Qc ?Ë
ær@U?¿œ{Ì)8Þ?ò±‡Ìè{@]Ȑ'*?ïÒ(ŒD¿Ý*qB¸a[¿ã'<"pj¿à@ÛÈRé¿éÿ-!¡:x¿ïõc#»ÆëAGNbll3FGL J1705.5+7134GB6 J1704+7138?ïÄcµî>?´Æ|qÅ´
?}Î% ý¤Ò?´Æ|qÅ´
?ïô'	c¦?X
ÚN•I?Vûí«ýdé?X
ÚN•I?ïã[ßϳÝ?oõý׶|«?l¤üb?oõý׶|«?ïÛrê$ÃÑ?R
o™³ÍO?rFŠÔ0û•?R
o™³ÍO?ï÷5Âã?R·Ò×<?Qû"…WG?R·Ò×<?ïÒ¯kN=â?v²™\=[Á?v¨Jw͊ñ?v²™\=[Á?海ꇕ-?†Ê²Í9‡ ?…ž…Z«Þ?†Ê²Í9‡ ?ï~|–Ã?I?sJGö"ï?0m%àHÜ?sJGö"ïAGN4FGL J1705.4+5436?澖iՏ@B~¹ÃÌîÀ:Õ3YɟòÀ<΂€x`d@ <–Þ(i×?üeћh¦³?ÈzxJB?ÀFí9Ô·þ?ö HZå?ÿ{=pxãì¿ëÇퟫ+'¿ÖŠmÂ%S÷¿Þ]*¸b2¿Òg"ÄËL¿åè4ÂTxÓ¿ÕpÏØAGNbllNVSS J170520+543700?ïýýÚ
ø×?#¾Iv…?00Z?#¾Iv…?ïí=.£pL?hwP«?bÂуSî?hwP«?ïðÜ.¹›?_y‰?¤?^G¤\}ÈÅ?_y‰?¤?ï¾SC/:ç?`‹ÙC&µ?€k/<`$?`‹ÙC&µ?ïù&{ò?I2	 _£?Kóe5–D?I2	 _£?ﻔțÝ
?8S,ô'ú?ÍÊòVÈ?8S,ô'ú?ïðïçâ…y?hÌPMdÖ?^ 0^°ý?hÌPMdÖ?îá/ÏjOÄ?‰¨‰ç"?¡íʟ¾?‰¨‰ç"AGN4FGL J1705.5-7423¿í-—ÛÜè¬À3jâ¸Ç\KÀ;ÏO?ÙÀ<Û÷@=ݱ@#oÄ8(»`?ùŽ­\Äüõ?Æ_šYÝìÛ¿¬6^ø?çÐ3:}ª@'¹Ëé"¿ïþƒþý¡¿î¨§ž¿ô!?ïý6âjBê¿âÏ@Î&i¿åFß•e?ù<a°@AGNbll1RXS J170548.1-742240?ïþގ&…?Ä{֝Ã?"AìA$?Ä{֝Ã?ïô¢ÂôB?X#^¹§¶¨?VºzF6ø?X#^¹§¶¨?ïñÁž4M?Xr¥|ºZk?]æ}1ŠåÂ?Xr¥|ºZk?ïö¼2Slí?HLϮᬙ?R‡›â–…
?HLϮᬙ?ïþ´Z²u€?¼?2?$ºXoÙŠ?¼?2?ïÎäi¡"J?••nF«6?xË.ï.?••nF«6?ïóIŠ|_?e°KÉïX+?Ylêô1?e°KÉïX+?ïáèá3Ü?nk®AÎÙÑ?n"2´?nk®AÎÙÑAGN4FGL J1706.1+1000?ÊÅtFw@;åƒjƒ,À:?Ò?ÓT¦À<ãAƒX@¬åm¶@³@ÔÜeÇ?ÉȹAՍ?Ã
é!›?õf"X@ÙÛÃO˿ךLGo'¿ãZÛ¿è…tžtG¿ì3l>¼¿ïé!ACAH¿îÃøþ.ÂAGNbcu3FGL J1705.5+0948NVSS J170556+100006?ïüŒÕ³G¸?5"¥©7ô?;™S{ïk»?5"¥©7ô?ïåÈè¢@?tMü5辟?j7úï¾?tMü5辟?ïÑ	yj=û?n¶ºeôè?w{CQÀ:c?n¶ºeôè?ïé"#–®?PÇûŸ¥¤£?fkÜ55B?PÇûŸ¥¤£?ïùÿ?Ó?O¢_‰¨å?K´‰·Â?O¢_‰¨å?ïwÃŽÍä?˜êkÊýŠr?'¯Þ‰?˜êkÊýŠr?ïj(P3Ҟ?Òå½
?'ºõüõH<?Òå½
?ï'õ® ðY?|=>~ZÃÚ?B"Jyë?|=>~ZÃÚAGN4FGL J1706.8+3004¿Ø"'Œ~p@ALSóÀ;9ï•N±À<¥o@Î&@ŠM<žÁÍ@SÒDÛÒ#?ÅLLfn¿¡_w½Yoæ?ÜóD›:ƒŠ@ûÎíäJ¿ï5/øOó?ïþ¨Fۆ¤¿ì¢ì^b‹æ¿Ðì±#yó¿äC‹ƒS?³!Þ:øAGNbll87GB 170454.3+300758?ïùÁLŒß?]ǟT'?HúÐ̋mõ?]ǟT'?ïîê£T¦?dA²×Ù?a\èÌ"Q?dA²×Ù?ïÔDÁ·+6?v£Éáœzè?uݟ	q?v£Éáœzè?ïöA&œÍ?=<æ4,Ði?S}ËìÖ?=<æ4,Ði?ïËÉùÍz¶?z®p
ª?z˜á?z®p
ª?$
O.?ƒùödke?€Þýq`ª?ƒùödke?ï®í¯#!K?†tih
?"D"7£I?†tih
?ï¼=)oÿ±?tKŽß¯e!?€ðµ§¹·?tKŽß¯e!AGN4FGL J1706.9+4543¿ã«
-@Bo.ßç[ÄÀ:¯¤Z½»¸À<_8ö@*‰¹QÅÅ@Ö#£s7?Ëÿ.^b6?¶~³Ë?é½ F@iùY¿Û^Þ&'d¿è-ÝvV¿æÐ
>Vý¾¿ë!°9ï¿ï÷á&öå¿ïÿöµšAGNfsrq4C +45.34?ïþ¤¼"/?÷½äGè?%´=‡1ɲ?÷½äGè?ïôxáë?W—È›©+?W=Õ(‰?W—È›©+?ï鰔6"?_
ÜxΊH?fOl¤ãý?_
ÜxΊH?ïô]tû)¬?BM¯éV"?WE´vW‰?BM¯éV"?ïÿx¶;?CŽž-PX?ý¡ÍûÐ?CŽž-PX?ïÍJÉÛ^i?€…'ÃÒ ÷?yZ›ÿw ?€…'ÃÒ ÷?ïé6•=im?l',3¡Úf?fÉjÌ5zò?l',3¡Úf?ï»VYlǘ?oÁÑéc¨¾?*i—¿–?oÁÑéc¨¾AGN4FGL J1707.1-1931¿ïދê4Ö@(ü)¥ë·À:ŽEîÑÀ<.·~†îœ@éûéd2@,p¼*¾?Êdk9‰äp?Øà۞KÛ@¥þ9Vbã@Õýê&$¿ï¿,Ñ?ïþÛ<Òf¿Þõt,öƒ¿á‹B=è¿ï›Ð`U*T¿ïÊ1¢ˆ.AGNbllPMN J1706-1932?Ñ'¾¸‰o?Èݑ1&yÎ?çl £þ;I?Èݑ1&yÎ?×2noÒÔ?ÍÒÊ7à?ärfÈÈ–?ÍÒÊ7à?æF77=ž?±xÖÞý?Óső'"Å?±xÖÞý?äDé1:S?¯\Ma3?×v-‹ÛZ?¯\Ma3?¶xK$È_ ?µ¿2Ü"Y?í0ö›/úL?µ¿2Ü"Y?²yÅ{»0?Ãpþ"Ò?í®PLJ'Z?Ãpþ"Ò?Çj³Iy
?µ£‹zþì?ê%S=-¡¾?µ£‹zþì?À©Æwôq?°	º,Ñ?ëՎbÿd?°	º,ÑMIXED4FGL J1707.5+1649?íø¡ž?N@>VÌ¢Ûa»À:4¿û-2À<L¡3ß@üÀ'a@DZ¢ãÅ7?¾¬W ùå?¾·ñH'$Þ@f´A»Œ3@
Ž~ZÎؖ?ïÿÔač¿âá',"³¿àêŽ^}
ó¿áŸv¼Ï)¿ë5â)>¿ßÙÙ«Ø`AGNfsrqMG1 J170732+1649?ïø(RjÂ?F–yüN?O¿_2æ¹?F–yüN?ïãAÞ=—?s÷›7•v×?l¾!µÈ©q?s÷›7•v×?ï–Kb÷=†?ˆQ~@Ûd?Šm'Lrl?ˆQ~@Ûd?ïȑiIo¶?`?z8?{·KDš¹R?`?z8?ïÕnlXÂ?vP€jXl]?uHÉÞW?vP€jXl]?ïnýÚiv?©R_þ€>£?' D±nå?©R_þ€>£?ï[oT¡—ë?'NWDX¡?"'o<ž£?'NWDX¡?ï9Ø¢T9y?€ŽÍ8†œû?˜Ä뮙˜Þ?€ŽÍ8†œûAGN4FGL J1707.9+0016¿ÒïÙ
!ü@6ü{þ~ÁÀ;‰‰¢À<D]­Z@¾@ Åå،s–@´ßbцp?Æy§¡D2࿔è:D')î?Бz{Ç »@þ=ìʙ?âziR©ñ¿Ø'-¿€Þã¿ëÁ
Áú᳿˗)gW}¿âòÅ_E4è¿Öi:@ԕAGNbcuNVSS J170744+001750?ïþ"øN'? [8v‰¥›?'°|û*»? [8v‰¥›?ïáß&@±?vÒw$²c€?nr р>•?vÒw$²c€?ïÝø¸ÛJ¶?uá÷Xrý?q£¢(ØÀ?uá÷Xrý?ïþ—õ]B?ãrW8M?.¦ä¡²V?ãrW8M?ïú·¡lvÌ?FQ§x@?E!yP´Õ®?FQ§x@?ïIŽá§Û?¨×…0ÇQ?–Î#Ë"¬?¨×…0ÇQ?ï×Սvܼ?~(¨Þf?t9JÀíÂ?~(¨Þf?ïøÖÇ]³K?BΘlŸá,?L¤á¦&@%?BΘlŸá,AGN4FGL J1709.0-3525?}'¼59ð@ŽÆ±À9ºâP3À;wjš¨@uZê²@f'amÙ!?ÑiIºß™?׺@Ù$@Y¾L×I(?ûÉTZ[:?ïß(Ÿ[zz¿æI]Áý¿ãù±œÅž¿çޘÜÛ7Ê¿êMDƒ½¿æóï»åüAGNbcuTXS 1705-353?ï@|;(¹Ì?]—ÍÌ ?—ðx¡Çþk?]—ÍÌ ?èš?ÂÂ8fÆ?ÌE‰_å™?ÂÂ8fÆ?ëŸÎíÁí~?¨ÜXlb0?Á€ÄHøJ?¨ÜXlb0?ërsȦ0?¢ÖÜö.©?Â60íÍg@?¢ÖÜö.©?èsò–"ˆf?Ã'ˆäs:?Î05¥±Þh?Ã'ˆäs:?Ç\c
ïл?Êëá©Âu?ê(ç=DÑ?Êëá©Âu?ß²}¯òæ+?º?	b Ó×?à&Á(Œë?º?	b Ó×?ÎëUók`æ?´È£Jnúd?èE*ƒ%'Ç?´È£JnúdMIXED4FGL J1709.7+4318?ç÷LÔ*Jh@BÆâ¨eÀ8dVôÙ[À;ÑLF)¯ý@¶Ò«@Å}?Æ¿m? µ"â>?¸¦‹€¸]e@ŸAò×s@nE­ß â?ï¡Ä«–`¿ß!æúËb¿¿åƒC…¶ä¿äÓkL4"¿ér†áa¯¿çƒÐ¸ò$AGNfsrq3FGL J1709.6+4318B3 1708+433?ïö˜w§ù¦?P'HX–?RÏ­MØ?P'HX–?ïî¦ô ü9?i
ú_DB¬?aYkb^x?i
ú_DB¬?ïÂÞ%ÝÄ?'Ÿ2öMà?~íŸ&?'Ÿ2öMà?ïþ×给&?ª«÷ðæ?"'}å?ª«÷ðæ?ïò: ô?V5Qïy?[å'=wS?V5Qïy?ïÂ:.œm?†ôÜÑ8æ?~âèÂGŸé?†ôÜÑ8æ?ï¹Àgª?‡Ã>
Õ?ùä†Gš?‡Ã>
Õ?ïýÔMü¥?%—²Z­ÂÆ?1]—ƃ<?%—²Z­ÂÆAGN4FGL J1710.1-2030¿ì5»Ùèò¦@&°Z-rÿÒÀ:¥P¥4À<(äSÒ,@bBÁñ@ÐAÌS*?Ëü¨>O?×éw}e"@o?Rü&W@M™¢Rû¥?ïû´a"ñ¿åd8>4îõ¿ÈFû&§^©¿çŽâá·ª¿æ÷mT—1
¿ïÿW~lªAGNbcu1FGL J1709.8-2026TXS 1707-204?ìB͸®2?Ì Gü¡"R?½é';'Žt?Ì Gü¡"R?æÖ³xña	?Êl'kÖEz?ÒR™=í?Êl'kÖEz?ìÔ
+jD ?¢©öîeL+?¹_–¥÷µ?¢©öîeL+?êus–òí•?¡¸4¯øM?Æ*1¤4I«?¡¸4¯øM?ëÒ,AÉÆU?ƊB~Q?À·NøØæ®?ƊB~Q?ÅK§ûF?ÊDzb#œÎ?ê­?V>n?ÊDzb#œÎ?çÌ3ÄA|¼?¶(Í;_8?Ðg˜w}ˆ?¶(Í;_8?ԏ7,´`g?´ÙV­Õž?å¸di¥ÏÍ?´ÙV­ÕžMIXED4FGL J1710.3-3943?ÁødçF†Þ?¦Bî"n%3À8@‹áJÀ9îÐè»?Ý@ܶlŽ@Ásûz_B?ºÉ³<ØÎc?Òê©â<Á@¶8ݗl@–f‹û r?ï¯Çˆp|?€œ ½­Ó–¿â‡ÐCyÒ¿èöN¦V@¿ïi˜¾&A¿ðAGNbcuGPSR 347.050+0.041?£ÀcÍxÑõ?³t·TCë?îÃùÃ61Q?³t·TCë?¾/Ác¸J?¶žÞðc?ì:ӈþ—?¶žÞðc?¾e·ÿœi?®|,æê?ì3N	s?®|,æê?Äp/¬¯»?¨!ä"S^–?êý#ôÔ?¨!ä"S^–?‹èVæ͜.?¸/!ðY‰?ï^¤r‡ÿ?¸/!ðY‰?ˆorƒÊG?+Tglh?ïžB5ãs?+Tglh?‡T2ap8?xl{²2¬¢?6±9k?xl{²2¬¢?oGóáòú?^¤K;w+Y?ïàñ¸G7U?^¤K;w+YPSR4FGL J1711.1-4600c¿íEýœÅÞÀIZ¼äø=À9œR3©z¸À:µs¯ûî@ÿö¿ºj @i½@gÏ?ךŒàŸ?םŸQ>Œ@ÇOšr®@®ÞzIG¿à7(áÀ?ïÿÕ"[ʁ¿ê­ÂC±Ü¿èV° Ï/¿ïîõÁ2e?ï
•ö]AGNbcuAT20G J171106-455254?ëE5ÈJb?Æw]®:?Âë(Þ×¢z?Æw]®:?éMnÙZ,z?Ézåð_N?ÊÊDš—N?Ézåð_N?çhUÛ:	!?µh¢†Ì93?Ñ/TI‹í½?µh¢†Ì93?ëÒ¸ãЎ<?°É%3?Àµp½Ç?°É%3?æ*½í¥¤.?р@ÙKÇ?Óª"$´·¥?р@ÙKÇ?ÕÒ$qñ¬?Ô¢ÉMÄâ?åíÇ*?Ô¢ÉMÄâ?ßá,UH‡?¸©zfÍ?àqiÕ[½?¸©zfÍ?À J¦9æ?¶MX$¦Ÿß?ë÷ízq‡?¶MX$¦Ÿß8MIXED4FGL J1711.6-5027?åF/À¶#À؏>ÕÀ9Z`ȗ³æÀ;mcr–'@BDmÃ'@WS£ìó?º S7
?³'T®ƒ
·?øÂ+‰Æ@t&µ÷HK?µëî>ü-ý¿Û2¼`¦¿ê©ãÉh">¿â'¾@—õ«¿îo݈†Í?Áê}ø(p7AGNbcu3FGL J1711.5-5029PMN J1711-5028?ï÷6Jiۑ?Kϳ0Ú§?Q"kËþf?Kϳ0Ú§?ïßä]y?ÅÏÕ°>(?pp
ð]¿‡?ÅÏÕ°>(?ïEÜÓÄÒ?¯(bA5?—\$bÉ·?¯(bA5?ïÞrÈä#Å?WҝÉåt?pƛ"iT?WҝÉåt?ï63ï¬ÜÔ?¡· G?™9'
deŽ?¡· G?ïÑ_P?¬¾ÐTÌ?œåÔ$èz?¬¾ÐTÌ?í|㮙8©?§úªF3AÖ?´⋤.5?§úªF3AÖ?îÆK0úŒ?'àÎv&?£›Lûoó9?'àÎv&AGN4FGL J1712.5-3142¿Ô#ÓM‰9"@«½À9ÁöBçÜÀ;2H˜F@®Ÿ]'ùC@be+ÓÃ?Ñ|Òì™q?ØѡȽ@²q¼Û¾?þœyGêz?îÄ!ÝËLÅ¿ÔfˆË<¨¿ê§(-E³h¿å¼þùoÿç‹5ó×ӑ¿ïÿõ^'AGNbcuNVSS J171309-313912?ïu°Xîó?"%5æä—?'Iÿtâ!•?"%5æä—?è×ú8?ÅþýmöË?Ï°£¬¬?ÅþýmöË?ìU!}?©ÃC'(š?¿õV÷¼Q?©ÃC'(š?ëöÞÎNy'? ÊÔF‹!(?À$"ÆÆø? ÊÔF‹!(?ê]k|¿ˆ?Ä{'«7E?ƊR
ßî?Ä{'«7E?Çå¢(*ä?Ë'æA°
?ê:ƗuõG?Ë'æA°
?â•|U³]2?»Yj]œ¬?ÚÕT™E?»Yj]œ¬?͂Ê9
?¶kš·¡£q?èŸMq¼Ÿ?¶kš·¡£qMIXED4FGL J1712.7+2932¿Äøà¤Î‰™@@t`$-À:HOžÀ<e$îÌÑÕ@ ˜V]¯³Œ?ümfL~?½
ãÉ­?ª$÷A{±?𨯠Ä?õeª^Ôê¿ÚIËÛ¶µ¿áh¼""Õ¿àXa@ß¿Þ~+ÿã$¨¿ÉI"ƒ\ì?¿Ú6›¦AGNbll3FGL J1712.6+2932RX J1712.8+2931?ïïm ¿¾?n¡L¬I?`ó'×1ð?n¡L¬I?ïÖ"®»?1ªjtÚ?tð¶ŠåÒz?1ªjtÚ?ï³¢‡‡{è?†5Î`N3?ƒ^}í?†5Î`N3?ï¢6t—gÌ?pÉLº;?‡rbÌgœþ?pÉLº;?ïäðh™'¯?c"Òh¿Es?k—'y?c"Òh¿Es?ï€kdî?¨¤B<Ö?œÏò•5@?¨¤B<Ö?ï³,aK¹+?†‡·6;?ƒ4ç¢õ]?†‡·6;?íüÁ7©uÁ?›	Œ¬ÝTk?°öCþ,w?›	Œ¬ÝTkAGN4FGL J1713.7+8844¿ä1»iM š@;¤ß&k¤"À;Œ`b@føÀ<ìXJCðñ@!aTБÓR?ûNB¸â4=?Ðë}&œKü?Å4á^)V?öžÜd…@Ó~Ì
à¿ïÿÔÌuŽø?ïÿ®XëT¿ÅZF@+>¿¹\èä/"î¿áŠ!¡»Q$¿à…ïbùÊ\AGNbcu3FGL J1711.6+8846NVSS J171602+884416?ïý¶‹ås?+&ÔÂp?2K¢<kÆA?+&ÔÂp?ïñþcâl`?\'ìñ:ÙZ?\8« 
?\'ìñ:ÙZ?ï龛ÂÏÚ?b$+ìâ}Î?fAdöE?b$+ìâ}Î?ïåa.KËc?MºŒ
iUN?jžÑÕ0Ü´?MºŒ
iUN?ïü‡l	W[?2zÿ›x.?;Ä ¶ŽIV?2zÿ›x.?ïǚ?|öøXbŠî?|2ñoõ€}?|öøXbŠî?ïÝâð`áÓ?tÑÞOM'?q‡¶Ñæx?tÑÞOM'?ï¡r[1Ý?vù¦Xq–¨?‡£)3ˆ¡?vù¦Xq–¨AGN4FGL J1714.0-2029¿ïò½¢ÀèF@%4f+®´À:N{.t‡'À<
-€kË@#ÿåSƒ?ùµ(Ö¸ÞÙ?¾è(råЪ?Žtøì³?Òñ£[dT¾@	¼IGǕ¿ïÌR>[î?ïýð@o[Ø?¡K'_¯ª¿Û¼J~Sm¿ÑMR-Ê=¦¿Ê÷µP-ëAGNbcu3FGL J1714.1-20291RXS J171405.2-202747?ïüíè©?Nr¯Û¢Þl??'Êå/?Nr¯Û¢Þl?ï¹Ãw°Ýû?™/S§2cž?"1{<?™/S§2cž?ïË»4žî?}&ž(¢?z"e–kì?}&ž(¢?ïù]õ‡3Ä?::Ó1:ö?Jˆ)ø¡³?::Ó1:ö?ïú°?GÚ¸C?Üø?DEI¦úS?GÚ¸C?Üø?íŽß͖²p?½k[`×cÝ?³‰'n…ƒ?½k[`×cÝ?ïÀO©
¥Ë?"òÍÿ$…?Ø+d¯šs?"òÍÿ$…?ïô¢sN?JüøT‹*À?V»È²Ú?JüøT‹*ÀAGN4FGL J1715.0+2616¿Ðªb® @?×a»úìÀ;ú61ëÀ<uÌÆ폻@÷ݜ¨Ã@y'½µÕ?̳€u†>ô?¦6ÌoÚ®b?ÔÏí~<Q@j#¹?£R~ÁÀÃï¿ä±À¢¿äþh›Œ¹¿â-t½l1¬¿ïþ*½ÃÅg?ïæ?šIÂÂAGNbcuMG2 J171454+2614?ï÷q€öµ~?Iz ô,<?QþÕS?Iz ô,<?ïê'v#?{'·¥bÃ?erØÁÍí@?{'·¥bÃ?ïÄÑ!+"ú?w)Ó[Æá?}—oN·?w)Ó[Æá?ïñ|2ð1?F˜ÚÛñìa?]š*œŒl?F˜ÚÛñìa?ïõ/LHØâ?Vš'¯néÕ?U¡g'
,?Vš'¯néÕ?ï±¾)­È?‹?€EÖ;?ƒuœLñÝ?‹?€EÖ;?ïÉ·NéМ?€ >x"‰?{$Xx‰Íø?€ >x"‰?ï!k"6?|òȝ/Ö¨?Œ·¥MuâW?|òȝ/Ö¨AGN4FGL J1715.4-4025?ÁÕ­Pۏ³¿ò"ãw3=DÀ9Øc—À:ð}e†l–@ x>fB)E@ð	yü?À¦Th-á?·vÀіá?ø ­Ú™>*@jÆ?ïþü—åº?íØ@|g°¿å†\Û£)e¿Û‡ôU§ÒB¿å"i£ÙŽ¿é»ÃŽAGNbcu3FGL J1715.4-4028PMN J1715-4025?ïúx­¡õo?P`›XŸc?FINb7Ë?P`›XŸc?ïÈ°weù?†øcyX"Ú?{§ò(Ð#†?†øcyX"Ú?ïC齄–Ž?'£'­m+À?—'ÈKý'9?'£'­m+À?ï´n4jb?n.Æb•?'ä_§Ž±€?n.Æb•?ïòà°?µ?`yGnÈmi?[ð>üõöp?`yGnÈmi?îÅ(Àµß˜?´4Vº%…?£­sõ}í'?´4Vº%…?îªIæºþ?œ÷9ª="B?¥[aîÄ&?œ÷9ª="B?î­®mªí?—ƒ'^¶?¥%!ᒇ?—ƒ'^¶AGN4FGL J1715.8+2151?íÎGfÿ@>HèÙrÍ}À;!•¥ïrÀ<Ž*pìÒ&@ó}Ë$@–U&£ø?ÍÕLù	ð?²8ÀxÅR?ã1&¹@(@"Üç÷öq¿ÆU±7pÉ¿æm¢À^ÕM¿à¶8 WäC¿èRˆÎp:û¿Í÷¤¼¸W ¿ï÷ÔCédAGNfsrqB2 1714+21?ïøfFcš7?^TÚÉ¡ár?NfåõXxˆ?^TÚÉ¡ár?ïèAê¨wO?ol¼ Õ?g¾0÷?ol¼ Õ?ïÎ[Nc?uù§
"ÿ­?x÷ó`Ç*u?uù§
"ÿ­?ïñ–tsH?Cø2WF]?\Ó¦"0²?Cø2WF]?ïí¸+nÝr?`‡ùzR?bGÔD•ó?`‡ùzR?ï›i–vq?'·«H/Ô
?‰%¹ÑÿÀ?'·«H/Ô
?;"?‰ÓÃ[®?‹R8&Ðò?‰ÓÃ[®?tX¹Í?{v2<:0?ˆ›b߂¸Ö?{v2<:0AGN4FGL J1716.1+6836?ÓkZšð@@áOKD¢À9°›±¡ÎÀ<qD…kl@$´o#@ðçä€G¹?°Od´Ëy?‡Ç8ä"(õ?ÕòoÀ@X%åí°?¼]ø®§ó¤¿â'f$!Gx¿ç2bo¶Ç¿álÁŸG.¿è7®ø¦ok¿áº>À//˜AGNfsrq3FGL J1715.7+6837S4 1716+68?ïþ»1øSA?€h̙è?$LÝö{š`?€h̙è?ï÷ƒŠ
µu?Uµ¡''hA?Pøë~à¦	?Uµ¡''hA?ïôΟ‡ö?TÌ
_'ˆ?VbÁ'úd?TÌ
_'ˆ?ïþÈ4·—±?™´å
&—?#|°Jf–&?™´å
&—?ïýÀæGÙ?*̾aà|Ð?1ÿj€Ӈ?*̾aà|Ð?ïß"•´»<?s.h½hŠ?pnµ+Ñ®?s.h½hŠ?ïèÍ#èE,?r|a•;O?g2ÜN´"Ò?r|a•;O?ïþ<Ó3Ýí? ÅTÖ²÷?,2Ð|{? ÅTÖ²÷AGN4FGL J1716.3-3421?ïhʋ\ž@ݨ!ò™À9X™I—À:½r`o¬`@ZO+â1@¶Ú@¨?Ä'îÆò˜8?ÎÅ3æ·Yž@v§&J@¥Xz—?ïԋ/Ÿ*¿çÇb\«¿ÙÏ QC¿r¿å\½p8w@¿éÄ
¼¤¡¿ïý"#–]AGNbcuTXS 1713-342?ícæ³l˜?¶isÊZµ6?´çØȬÍ@?¶isÊZµ6?î¦:>˳?ªöWì˜GŸ?¥œ\¯Ú?ªöWì˜GŸ?êË9‡5=ú?¯$š
8Ëï?ÄÓã+?¯$š
8Ëï?î`¸XãZ?'«À¤C?©ôz}Ùü_?'«À¤C?Ý/Û>Cvf?Ì«w^þ‹?áh`ÞDÍ?Ì«w^þ‹?çnÀ)Ñ4»?ÍC7ˆé"O?Ñ"¬]–‰?ÍC7ˆé"O?â²%¢YF?µ´lɸãd?ڛ´»Lát?µ´lɸãd?äˆ(·ë?¸`‰bi׊?ÖﮑÖà*?¸`‰bi׊MIXED4FGL J1716.3+3434?¡˜ÙA0i@@Òb^™éKÀ;·ÀÌ
Š,À=yÚ6AÛm@[ N@†A­
ë?Ó¡Fnªƒ?ïþ@_‰Ó@9¥e¶š?þïΔ£º¿ïëiÀú)?ïÿæ4|ßO¿Ïàœøɪٿì¬Ù¢s1ü¿éæràÈ,T¿ïVqáÄ«–AGNbcuFIRST J171642.1+343856?Ív'/FP?̖zi}?è¢[`4.l?̖zi}?ÔS:`_L}?Ét¬€¸2r?åÖbÏÐYÂ?Ét¬€¸2r?Þôöú"?·'ƒÝ$Ø?à…ø"'þo?·'ƒÝ$Ø?Ï,)õûM?¯×ñ\ì?è4ùõ'-?¯×ñ\ì?¨Ü)F`ì?¶<]Ïû¾?îr=kŠ+?¶<]Ïû¾?²réû×?¶t°,ãJÙ?í±¢ÀÅé•?¶t°,ãJÙ?ÆëÀ:(?³´W[¯¤?êE?ñuà?³´W[¯¤?˜‡a–*©?†‰z5ÒÕ?ï;Ä÷7ÑË?†‰z5ÒÕPSR4FGL J1716.6-6707¿ÛªÅ0KLZÀ0Q€¡{kÀ;<MI^ïÀ<|ók@•±êk@<î?äž?Í/d\ m? j‹Üdî?Ö²Üá—à?þÌmŽÎºc¿ÒFr©jÈ¿ãIÒ±é¿èg
À²ã¿Ä˜†t¿ì!€ƒH¿ïÿîÝÃÀ	AGNbcuPKS 1711-670?ï÷†_]¼&?D¶ç†@‡?PóA+ʃN?D¶ç†@‡?ïí!n9Är?h¼æ«?bޑò6ä?h¼æ«?ï¼7€lCm?}<֊dÂ'?€òÔõ?}<֊dÂ'?ïò£lðÝè?@SeÐttÊ?Z¹&xùߪ?@SeÐttÊ?ïø‰j2´ï?GžYeýÑ?MÚW	1C"?GžYeýÑ?ïÃó÷Ö]<?†ÄlJÀ"?~Ñb"?†ÄlJÀ"?ïÆbd'Q?€5-ÿÚ¥¯?|Îùãkz?€5-ÿÚ¥¯?ï îº³D»?wËÛÝú-@?‡ÄQVžm?wËÛÝú-@AGN4FGL J1717.3-6045¿íòM²1ãÀ)ížbV6mÀ:ïdDM6êÀ<•—rwí@6ƒºŠ*@mUhƓ?ːЇÂV§?ܚoÂۇP@=TT+
@jŒ¢:R¿ïð‹ž.SÐ?ïÂ{ƒ€¿ÖŸ§z­Æ!¿æ=í¡X«¿íĜý|B¿ïÿü¿ÙŸCAGNbcuPMN J1716-6045?î´§‡Ìp9?¡¶ÆôBGþ?¤µ‡€¥Gq?¡¶ÆôBGþ?í뽓Hò?±³5<-õà?°¢e¸k—?±³5<-õà?ì³t¥Tžú?¢š÷Py­%?ºdZÕ[1?¢š÷Py­%?î(Ù}ŠDg?Ý5Ü£?­rh*ËUŠ?Ý5Ü£?ì7ðVa-?¶$ê쮥¬?¾@}Lö—?¶$ê쮥¬?åܚ‹Ã(o?ÍoWhih?ÔFÊèy¯!?ÍoWhih?ãÒhƒo?½N–â–Hè?Ø[õË.ù#?½N–â–Hè?äêMÍNŽ?¸†¡Gî?Ö+debãÙ?¸†¡GîAGN4FGL J1717.5-8114¿é]B;eÀ7^'¸#È\À:–@
²
ªÀ<iqDæ¹Þ@×`]bÝ@ÈCæߞ?À»¡VQp`?Ž¥vLJ"?Ììa<°à]@íBDH.m¿é
Ï@Åm¿Ù́»¬i¿ä I·¿à^^…¿áü¦¯+Ò¿ã!R•Ï	¾AGNbll3FGL J1716.7-81121RXS J171712.6-811501?ïüBeõ?Iþƒ:
??Uî¯qÛ?Iþƒ:
?ïõFÁ¸û?WûÎî<@?Ur|¡G­#?WûÎî<@?ïô.qò$?JÎWxµÎ‰?W£¶â!?JÎWxµÎ‰?ïûVº™:ñ?+ú[e¼æî?B¥å؆Ñ?+ú[e¼æî?ï÷™u÷ç?JËbc¦Î?PÍ\	Áw?JËbc¦Î?ï͏û`3?—Kräõú?y83¹¦a?—Kräõú?ïõ™4Ío¾?f௷ûõÓ?T͖O#?f௷ûõÓ?ïéŒrX{Ü?W™?µ'Bb?fs"X?W™?µ'BbAGN4FGL J1717.5-3342?är‰lGH`@'ô}ë¾*À8:¯^&üÄÀ:[";"*Å@#ý:¨Èa@dc!7ˆ-?±LžŒˆ?Ã`à?›Ku@U£ãŸw)@4´g¦,?Ð87~òNg¿àÁQ'Ò­¿æl«ÅHg¿åðQ£"î¿ì›]"°§¿ã‹Ú"5¬ŠAGNbll3FGL J1717.8-3342TXS 1714-336?ë3G Ü¸?Å¡!$à,?Ã2á|Ñ!?Å¡!$à,?ï¡gï'–?Š·4gÜ?~¯LšA?Š·4gÜ?æà¨ÏlJ?²ì>¦§à?Ò>®a&ák?²ì>¦§à?ïîå^È?QTdý1!?aï½a ?QTdý1!?îñ."³ê?¡ùн«? í¹Ú?¡ùн«?í1ªilø?¼U»ô7u?·Vr®lf:?¼U»ô7u?è2å—ÁI®?²A`4xL?Ï4i úÙG?²A`4xL?ïFàힲ?‹òZuÎU'?—#âGT
?‹òZuÎU'AGN4FGL J1717.6-5154?²Q†È¤À "ön†ÆÀ9r"áÉ´À;x"íˆ.7@šU'þ@%!4y?½nýùëi?ؼ‹ ¯ø×@¯œ…×E@ 	%m¢Æ?ïû—áÂA¿ÙßND0±y¿çœ/`•Áô¿èÎ,~
L¿ï\˜AÒ¿ïš@¨f¼AGNfsrq3FGL J1717.4-5157PMN J1717-5155?í¯Óe?ªöÁ)4ê‰?²‡÷g"Û?ªöÁ)4ê‰?ïÓQM?‹äCQ‡ˆÕ?vyׂ–qi?‹äCQ‡ˆÕ?çT›çìQ¼?²½;±È??ÑVÈ0'\ˆ?²½;±È??ïî"|Q½À?PzEŒÁ?alƒœdG¦?PzEŒÁ?í–aô;ђ?«MΩÁ?³Lð^ýZl?«MΩÁ?îö-à •f?±SO:–M? #Ëbôª?±SO:–M?æ¹W÷&¬V?³Š:ieý¾?ҍP²§T?³Š:ieý¾?ïpúåÉë?ÊW†2ŒU?'à¿F˜?ÊW†2ŒUAGN4FGL J1718.0-3055¿ïíäŸ|\@7%€ÃÿÀ9<,†pÈÀ;Eˆ×ªva@–]Z#7@	•övê?º¿Œƒn_?µÎ–?`×Ë?û¼µ'•@ø§üaæ?ï}!"Î~~¿Ý]ÅB"пèw¦×o¾¿Ý*Ü·ü[0¿ç#ÑÌk¿çx×ì;AGNbcu3FGL J1718.1-3056PMN J1718-3056?ïù}ѫȊ?CNpá°?J¹ÄP·1?CNpá°?ï•c!–n?š» ÜWO	?Š§7ŒÀ4'?š» ÜWO	?ïÐ6,sÌ?z€ìK… ý?wäé¾;	Ï?z€ìK… ý?'d"ö?r¼¹¤ééD?Œ›q-–q?r¼¹¤ééD?ïèçŸr2?d•*š@‡&?gížfÅÍ?d•*š@‡&?ìó_9»&v?¿LxÐ1—c?¸e3³O?¿LxÐ1—c?îԹΠêú?›¸Ì_Û?¢´cñP\?›¸Ì_Û?í	[¸&f`?¢	I«ŸÊn?·µ"?:À€?¢	I«ŸÊnAGN4FGL J1719.2+1745¿ÐH£>ÖKô@<†`ÔÀ8®j}L\À;®z¯É‡@B.'åue?ÿwÓv4:?¤ô^¿±Žá?¸??ŸÁëŒ@_e©Oð@"µçØí?ÐÞ;Ÿ"X¸¿Üÿ"Év7¿à!,jº¿àÑÍmÜ|¿âÎHÍÏ+L¿èÛÑLŽNAGNbll3FGL J1719.2+1744PKS 1717+177?ïúŽÞC†?@яÐ{í?EĆ0bb(?@яÐ{í?ïàû]Xö'?‹˜œšñW?o¢².¯?‹˜œšñW?ïÏ^gòá?|RÄþk¯?xPËð'÷‡?|RÄþk¯?ïÿ¦ôa«>ùpEŒ¢øT?y‰ïC|Ç>ùpEŒ¢øT?ïûcSÑ'?9l×HÍhL?A¾rµ!Ig?9l×HÍhL?ï`UµêE?¬æj½?"õIDvåU?¬æj½?ïÓ4œƒž?'ÍùŒ
GQ?ve±Î¯Q?'ÍùŒ
GQ?ïÿH¦G?Ÿ³Ï÷¹'?­Þ»Búœ?Ÿ³Ï÷¹'AGN4FGL J1719.3+1205¿å+ìï@9ØÈÿ¸²dÀ:Lí=…œÀ<4•äÙ3
@!; ¨×z?þ"ÑH\$?»1)ÑW÷¿™I#W›?àä†&ö@RgÎÆL*¿Ò亼)¿è	ØÆÖÇ¿ã9Pïܹ¿ÕõúX R†¿Ý±ª|ÀÅØ¿ÂlF9Ë'ÜAGNbcu3FGL J1719.3+120687GB 171701.0+121016?ïüŽJþM?Tê·âߦ??£‹áôj,?Tê·âߦ?ïä'«QÂ?u—ãÊ1íY?knêŠH&?u—ãÊ1íY?ïóTüäÿ?aáT¥ÇÆ?YWîS-B9?aáT¥ÇÆ?ïõ£ýíùe?:ö¼-´}?T¸‰Á¦#?:ö¼-´}?ïù#ÉDe?@'^JSW`?KpÙ뭗ø?@'^JSW`?ïXǑúhç?ªŠ±æ•Á`?"ç
À²ã?ªŠ±æ•Á`?ïò¦Ó¾Ùo?føFX˜I?Z²XR\?føFX˜I?ïÕJБ[?d}Pž¤?uZ—¡Tøx?d}Pž¤AGN4FGL J1720.0-5101?ë‰L
¹jßÀ‰êpKÂÀ:^Òn¦À;~1ôo@ڋIõ—q@À¹Ü/@_?ä/IŒ;?è?üÚ±'Þ@ g–@ý¦oëË@?ï8S~,UÉ¿ájzÈ:£¿éŽ¬ l¿î`ñ²_c¿Ûn€m¤?Vérí)ÛéAGNbcuPMN J1721-5055?ívj'f p?Âc0Wqè?´L®ÄÎü}?Âc0Wqè?êŸØIÏú ?ž½†o¥?ŀžØÀ?ž½†o¥?ë;ÀÐ4Ç?¯ó¹íïT?Ãÿè¿,â?¯ó¹íïT?í±¼e¡o|?¡"­pdaÁ?²r҆¡?¡"­pdaÁ?ç‹ÿàuv$?ÒU{pþ^¯?Ðè?¸?ÒU{pþ^¯?É6ÆÆM¾?ÊéDŽc||?é²NNlŸ?ÊéDŽc||?äèÚ >Ü?¼7‹Ð‹Ñ¸?Ö/èK¿'H?¼7‹Ð‹Ñ¸?ÐQ}]p?û?È[pi§‹?ç×AQGà?È[pi§‹MIXED4FGL J1720.2+3824?ïöù#Aùu@@̴ἩÀ:¨–ùݧÀ<pÍ_™Ä@bl¤CÔ@͘ÚVù?Äíañ34?µ>M˜-…?é·ýgŸKŠ@Ìٌù£¿âSQ¶«ù¿ÄGRºb¿ê"'úð̆¿éâi·S¾Ä¿Ò+A!]s¿ïûÜàSúAGNbcuSDSS J172010.33+382556.1?ïù;.™?[RÞaY=1?KG~ =?[RÞaY=1?ïîâUcù?e*íg³?aópâ–è?e*íg³?︐ã²°?ƒ;'ƒÌçó?ÛÇ-|î?ƒ;'ƒÌçó?ïñE	õ­?D݊?]uí|¦`?D݊?ïºË"R»9?ƒè·mÀÿ?M7iAmÏ?ƒè·mÀÿ?ï¾´—æë?€lÒL?€RÚ®Ù/?€lÒL?ï`ôQÿ"¹?ŽnGÅâ-ú?"áu¼ŸÌò?ŽnGÅâ-ú?ïƒِC?€ùYDUI§?8;?M1?€ùYDUI§AGN4FGL J1722.6+6104¿â­ÏÝ)N@Ap\‰mÒÀ:2ì|•|ÔÀ<WÄ/oYT@n
I¯÷@š%™í|?¼•p•x?¶7¸¨þfx?õPû«©@8"XŒÞö?·äùibð¿è™‡+¿é‹K¿ì&+¾ß¿è!p}–ƒ»¿ðAGNfsrq3FGL J1722.7+6104GB6 J1722+6105?ïýÂ?=Š'3x̃?3{÷sÑ}"?=Š'3x̃?ïö[ë'³?Tma?¨'û?SH)ñµIV?Tma?¨'û?ïÏõÖRÔÜ?}þ ¤»º?xÚµ7?}þ ¤»º?ïú`Ã(""?2Áóµ>p?F|óJ"rX?2Áóµ>p?ïüXÍegÓ?<ÞàªÑq?=9"HŸo?<ÞàªÑq?ïÚ¨¶÷'?s†«ñW?r«û"V*ü?s†«ñW?ïÃBL"9Þ?'FQý‡'?~^Ùì#`ú?'FQý‡'?ïßþå«é?_‡ Ž¢e?p‡¨+‰?_‡ Ž¢eAGN4FGL J1722.7+1014?æ7žõ@8M¤-fkÀ8ù˜zµ¨ÄÀ;ãn)©G@Z×^K9å@qû9Ç¢?ªc,u)?ªÙ¿4¢Ž?þáDŽO¹@!O[?ʋîظh¿á!—à¿ä99±Êé¿âwÜ{~¿å¾´`šI˜¿âgƃ°AGNfsrq3FGL J1722.7+1014TXS 1720+102?ïýÈòlL?"/gÕÎ?1¾þ×þÓ¬?"/gÕÎ?ïߢ±Š?€o·"yi?p.§-æù
?€o·"yi?ïã;ÓYš?wú'kÜI{?lÄ, ã?wú'kÜI{?ïû*ӌ&?2ôè/…³?CWø=2d?2ôè/…³?ïûïA8P÷?6l¸‡gà0?@Bú×Ñ[?6l¸‡gà0?ï^Taß¡™?©ˆ'ÃÕ?"5s½,"à?©ˆ'ÃÕ?ïÕ®mï¥H?îú:"·?u(È÷¯<W?îú:"·?ïö‹Åùýe?G™"Iõó/?Rès•Ò¦]?G™"Iõó/AGN4FGL J1723.6-7714?¨ü:‡6À5Ë6žË2À8J¾*ršQÀ;Ÿ0µªq@¼n<c@t@ylÓh?Ÿ¡"
R%?¹?æàIV`@4·õ¥3+@
5"Š¶Ó?·ßW=ÿj¿á&B‰èK®¿ãX—Ü*7â¿ä'ô¦/ª¿é±k«¦·¿â.•3ÙKAGNbcu3FGL J1723.7-7713PKS 1716-771?ïø¤WžÞŽ?KPòӞ?Mn¢!3öŒ?KPòӞ?ïïï V.,?pë¦ä©5
?`ßv÷›ì?pë¦ä©5
?ïµ
3	¡?ˆ™n6ЇÔ?'½s?G%Ÿ?ˆ™n6ЇÔ?ïÿ(­-Ô?-¼—Æ?üǑÉÁ£?-¼—Æ?ïñègToe?^>|g"ž‹?\/1·VD»?^>|g"ž‹?ïÂ̗·†?­Ü¶h¡?~™´΢Ö?­Ü¶h¡?ïW®u§T¡?•|#^vO?•
1B~eó?•|#^vO?ïýñ셿?+D¨Îž­?4qvŸå?+D¨Îž­AGN4FGL J1724.1+3304?ïEÎñ½Æ@?»XK±À;$Ÿ¹šÀ<¿Áõv@ÄÑÞ¯xS@ȝ»gI»?Á××WjJ!¿µE@¦ä/ë?ï$8ž×ñï@½´«î±?èÚ>Oq¿î|b¡µÇοÇY¨‡s&¿Ó³ä¡Q¿á'óU͒¿Þj~yÊAGNfsrqB2 1722+33?ïúì‹À#W?@ùcuâõç?DMÐV} ?@ùcuâõç?ïð¨"ÔÖ?bÎdÉxšt?_þ®¿™$(?bÎdÉxšt?ïêmBèKÈ?q^–€5ø'?e'½Qm§—?q^–€5ø'?ïïnG†Qh?Cرlª?`'¸¥©—p?Cرlª?ïó Ä?UZV/†P?XÅفþª»?UZV/†P?￁O Ò?‡)°hî?€¬"L¬?‡)°hî?ïê•Æ·p*?u%é)Å?ej9…õ;?u%é)Å?ï¯ìuùE@?që®}Ä~?"âv¯ð*?që®}Ä~AGN4FGL J1724.2+4005¿ßTãéh@@'dobÀ9biAâù_À<RS‰êÐ@fëÇc×@§Ös>»ý?°ô¤9/Ì?ÁÔÀa.™@döÄíÛ:@Ž¦‡é˜à?'M
`!)¿â~€Ǒ$¿æ@&`¼Ù:¿ç—áìèì`æʤԿïýø‰9™AGNfsrq3FGL J1723.9+4004S4 1722+40?ïøŸ[zz?M`ÕBq?M''y™¼?M`ÕBq?ïóWø(_	?aÂHÚM_£?YP¯AîÚ?aÂHÚM_£?ïÒ¢M‰?m'Oì•R?v®öýg¿@?m'Oì•R?ïþƒÞÇK.?\¶ìPÿù?'‹¬|u?\¶ìPÿù?ïï)!êê?XÑM˜—Ä‹?`÷ÖüQ¥ß?XÑM˜—Ä‹?ïÑg&æÚÑ?yM¿ãµ?wLluå+‰?yM¿ãµ?ïŒït2?‰´\ä=žõ?ŒÄ"î½CŠ?‰´\ä=žõ?ïü8¿Sr?07)QíÈ?>:Ó]¦˜?07)QíÈAGN4FGL J1724.2-6501?îÙW	Q7€À/Ç$ p¸ÐÀ:¹n$ É9À<DçԐ@8O§³
@ê/~r̦?ÅÕ^fWM?£GPCۄ?Ý܏¸oH?÷<í–ÆÖi?مâ,°b3¿ê~íEé]¿èS¤Wb½d¿âr‡ÂÀð¿ä÷ÞþþxA¿ï뒠+.,AGNrdgNGC 6328?ïû¡nz1?H1˜b´?AzE­­ìá?H1˜b´?ïÐ=çäw±?… 	½qz?wáþ¥ß»?… 	½qz?ï×*eэs?kŠœ/ì…?tjÍêrp?kŠœ/ì…?ïØwŸì?We>¡ƒÏ?sÄ0ußB?We>¡ƒÏ?ïûA•Ý³‹?>åRîýÊ?Bù§¦±û??>åRîýÊ?ï Ü(µUã?®V‹š•?›äzçu¬?®V‹š•?ïµ~öf_l?'(Êß?' BWùÉ(?'(Êß?îwkã¡j?•
½þ‡Û?¨‰AÇE…c?•
½þ‡ÛAGN4FGL J1724.9+7654¿ÒãÀ™¸£J@?9¦ç_ö
À:¥ìeïH"À<^n£KÊ@¡@-lŸ»@¦;îך?Å0‹x™™Å?Š,†==ŀ?Â{R'L@	1‰èv¡r¿Ö5²ÿÇ ¿ç$w®G¿é¢
qÊÛ¿å`ø0'æ¿ãÔÄ}ròf¿ïÿïn¸D€AGNfsrqS5 1726+76?ïþÞðeÙ#?<×jæn#?"ûæø??<×jæn#?ïö«jHëy?U¬w·©?R©+³¯*?U¬w·©?ïð
ÌâœB?]ð¦¢<ê?_êfÄ7Ûl?]ð¦¢<ê?ïü]þ&о?%Í°D¢?=ZÌml?%Í°D¢?ïþð¾n,?!½¯&*¥«? ôí¿²^?!½¯&*¥«?ïØN0m8Æ?th¶ñ?sØçÅDô?th¶ñ?ïèäóµ?jO†Â{¶í?g
>ƒP³?jO†Â{¶í?ïêqÎN'?Uè]"¼?eŽ1ì—.?Uè]"¼AGN4FGL J1725.0+1152¿í"­éª@8yLýÔ»À7éÇ88U²À;*µ[–ÿ‹@°\ô͜Ö?ü@—"ìck?ŸÃËØlNn?®}£;P[@Öâdä†'@
s—ý7N?暴f¶î>¿ÝЎÃ|Áò¿ÜWí'?2E¿×QDX­¿à"$݅Û¿ÝÃÎ ‰ãCAGNbll3FGL J1725.0+11521H 1720+117?ï"þó÷š<?¶Q¿³êk?‹C×àè?¶Q¿³êk?擄߉'?"(ýf?†ÓÈL\{?"(ýf?ï•e8بg?ŽÜ£
ô{?Š¦±×"V-?ŽÜ£
ô{?ï2eúU?'!bÙǏª?™³@À¬±c?'!bÙǏª?ïóÒm¾?Y·#‹w?X[&:ØÀ?Y·#‹w?îŽZhM¾œ?´âÍV×Êy?§Y|Ûä;?´âÍV×Êy?ï‹›~îj?‹|Çè¿?9™ De'?‹|Çè¿?íz:k‹¿;?¡~©êyÏÝ?´.,¢X+¦?¡~©êyÏÝAGN4FGL J1725.4+5254?ƛÿ~¿'k@A
ïܜM©À;°£µ|N/À<Ó¿jäz@ ¬Í÷ó—@"0Ÿ<¦?")JÒ¿¶9&ôŸ?õe=ð%—@ŒUðLƒ¼?åãÉjÉø¿ê¶u¨"ÉY¿æ­}±Ü†~¿ãÅ6jö ¿Ø6]_+´¿ÆŽån.\AGNbcuRX J1725.3+5255?ïü}JiÁÌ?2§™'Áo?<«ÛŠ¹?2§™'Áo?ïðx,PYÎ?`¢Á9´jJ?_§ӎ?`¢Á9´jJ?ïñl<FàÃ?^'÷/=,¡?]'‡¶öªI?^'÷/=,¡?ïôÌFPW—?Cæhô;A?Vgsà' S?Cæhô;A?ïøá<4R‡?GE<·e&?L{'£K?GE<·e&?ï¿Ä‡j(N?ŠC"ç?€Þ)=~w?ŠC"ç?ïõÀ
"ú?czE2e‹&?TëH¿Â?czE2e‹&?žª?ƒê[‹¾{?Žžz´9§?ƒê[‹¾{AGN4FGL J1725.5+5851?ì¦ir@@üšõºÀ9ó+w}À<'\ä¥6@O²×-Mì@g­Ãó	w?±ñOŽÀ?žmã;åŒ?ë?N_¤@-2¢""ø¿àžóu®¿ácAM¨)¿äļþ"°.¿Ý»¹^Û؃¿ç
ŸàÛwŠ¿áM20±ÏAGNbll3FGL J1725.3+58537C 1724+5854?ïþ®±%HÜ?ÝgޔŸ¿?%ë×
å­?ÝgޔŸ¿?ï÷y—#PE?SҒÂ6‡+?QÑN+§?SҒÂ6‡+?ïù#UMB?8/Çà£È?Kr©ä*N?8/Çà£È?ïýrúsy?"Ò$?L;`?4h,4?"Ò$?L;`?ïþN©J*Š?!à5Y—ŸK?+m¨zýw?!à5Y—ŸK?ïՀ~PÏ?{H½<Pm?u?À·L&Y?{H½<Pm?ï÷Â.c?À?Y'v'å"_?P{£¤´N­?Y'v'å"_?ïúβwƒg?9B¶Ì/\j?DÅ6í[Dk?9B¶Ì/\jAGN4FGL J1727.2+0644¿ÞàŠ†x¡õ@5ÇÛLÂPrÀ:†R{ÍÖ¸À;ݗkÖ@ޛÇÇ)u@—¬úŸmï?ßB"úùZõ?åðBrÁ>?ÿË.LC¥q@	$á‹Ë¥°?ï/›™N?¿Ýsdѐ׿ëmµz °¿ê3­Á錄ïÿý¥\Æ?Ü×æ¼5CAGNbcu3FGL J1727.4+0634NVSS J172720+064123?ïꙫ&?}õ'Kž7?‹þEOFb†?}õ'Kž7?ï ßaW'j?•(§±7ڈ?‡È'°úÝw?•(§±7ڈ?îPP­õú¡?šqËȋŒ ?ªúõ ñ?šqËȋŒ ?ïŽP(#×?sz%"ß	?Œkõí8šT?sz%"ß	?îûr!Z˜¨?®…Ø¡¶+r? HÝíÆ~?®…Ø¡¶+r?íÂ|‡ÿ­?ºB֋´Ëñ?±ïL4š?ºB֋´Ëñ?ìþa«õ?ªRKþ
{g?¿¼ò W?ªRKþ
{g?좰¡ôó?¥˜֙
ß?ºêzóXh?¥˜֙
ßAGN4FGL J1727.4+4530¿å±P"t:Ý@@¥‡+À8qq¡-ÒÀ;ÿ+Ü&Üä@Jž5àŒ@'eŸ—
? p·ß;¢?µq"Q³ÑÔ@?Ø2\@|Ë¢Ö.J¿È+ç—rx¿ãšG>'òŽ¿æýdQµ¿æ­ÞÎW¿ë#Ÿa¯g¿ïÿÍ'ý AGNfsrq3FGL J1727.1+4531S4 1726+45?ïô'•û:°?K»yÝñ–?VÜÓ·S?K»yÝñ–?ïñ"½ðC¨?e Ó\‡?\փžG`·?e Ó\‡?ïÁüûrU?{t^ÚsÜ?'Óye?{t^ÚsÜ?ïýb£°–-?'([¯?4êâÂ@¸?'([¯?ïø²zªÚÎ?BåÝßê&…?M6'Î?BåÝßê&…?ïÀ¯êá,M?˜Ê\é·m?¨
¦Ç1‡?˜Ê\é·m?ïãdÇ2?x?òeûb?lû›3Ne?x?òeûb?ïùuُš?A½se?J(š;Ž
?A½seAGN4FGL J1727.9-0654¿ÝÇTÚÅ*c@. ½ì_9KÀ:AíHmÀ;Œ¿®Xë@±F ù4_@Õ%t.?Ë*"<m2?ĈSvÀ5?ú§ÇúÕô"@V½sé[Ï?ïýª R¿æ‰ùž<°¿ã~ÊuÚw°¿å¢>ƒÉN¿ïõ}$îÌÒ¿ïë%@@AGNbcu3FGL J1727.6-0654PKS 1725-06?ï/ôZ8
k?¢0f ܞ›?št°gL§?¢0f ܞ›?í&¥Âá€R?¸'ð·Úï?¶ÊÑèr?¸'ð·Úï?íM!żQ?¢LHð5Ø?µ–ñÓÕE:?¢LHð5Ø?íXNJ!?"ÌÑã¹½?µ?íÔ¸˜?"ÌÑã¹½?ê=̶žÚ?ÀЀå²e²?Ç÷Í%"–?ÀЀå²e²?âf:z,õ_?ѐú€±¤?Û3‹¦B?ѐú€±¤?å@üš£by?¾ÛGÛ%?Õ~ʹ;?¾ÛGÛ%?áÞ4v)R	?´Ñ#`¼µ&?ÜC—­[î?´Ñ#`¼µ&AGN4FGL J1728.0+1216¿îÜ(̹@7ùSÞ¤e¥À9,ÂËÂÀ;Ì4–	Â!@¤é
ìî@qÈâ\?±\Á! ?·›‹¡´EA@³¼?¶Ï5@€'4Í<3¿à#Cf‡–¿Þ
D<œ¿æcˆ€l¡ê¿æk:ÁG¦¿êœ€iFëw¿×ú ø2¬AGNfsrq3FGL J1728.0+1217PKS 1725+123?ïü2¯:ü¼?1Rs=Z?>jˆ$K?1Rs=Z?ïÞ="dŸ?xì×3Îþœ?páoz|;?xì×3Îþœ?ïсºª¶M?p‰»X?w?"'—•à?p‰»X?ïóò?ðR?Eõ-Ÿ»"?Yüþúœ?Eõ-Ÿ»"?ïñ°xû‹É?Woº¸L1?\Ÿ
õª=?Woº¸L1?ïT†ûáh?¬³LþH`e?•o ŽÓ
?¬³LþH`e?ïEiL…û¾?'õ@¯Ý#?—RÖpøV7?'õ@¯Ý#?ïÇÿÝ_0?iÒ«¤±'?|p´SÊ?iÒ«¤±'AGN4FGL J1728.3+5013¿»f[ã@@ÄÁæ¯ÍÀ8'û¡ÌnÀ;·–5df@ Ïÿ1N?ü%Ê_4Bþ?Ÿûß=#?ˆæ2	Μ?ê{`ž{V@Â
Җæ6¿äŒšþ§±¿à:þƒ©¿ßý‡[ח¿ÐþD4ã¿ßlL#Å&¿ÒèoÀ';¯AGNbll3FGL J1728.3+5013I Zw 187?ïÿ+ ±®?GÂ#|è?‹íHr`?GÂ#|è?ïö]sòS?TPšøÃc€?SE\Ù?TPšøÃc€?ïæ#3r?xÈ<ô—áò?iÜ̖;9?xÈ<ô—áò?ïÿ˜	²Âq?¤ý¡¾´?	ýŸº<?¤ý¡¾´?ïþŠ/KûŠ?(s¿êö›ö?']¥)´?(s¿êö›ö?ï×waF¨?wg-˜·ïâ?tDO^»¸Ú?wg-˜·ïâ?ïã½oÙú?}79Y]2?lôB±"EÔ?}79Y]2?ïÿ§·X`-?ô–À˜W?"J+?ô–À˜WAGN4FGL J1728.4+0427¿âI>'áy
@4w%_5½À9†…˜ZÕ9À;®MnGÜ8@Øõ¥@x<¢G¾?¸á(ypÚ3?ώLßV½&@Q\þØ<@Š³áŒ?å÷$+Ž¿ãs…ô¡'¿èc¾yå¿èA~O'7Ë¿ïéÈ@K·¿ï¸ 7­ì7AGNfsrq3FGL J1728.5+0428PKS 1725+044?ïEÆí ¦?'ÃáÆÍè?—G"_m§7?'ÃáÆÍè?ïrk~g±?Ÿ8šFǨ?'²œ'œà?Ÿ8šFǨ?î­çõ¥¼›?–Mm:"ã?¥!€¨7ëI?–Mm:"ã?ï‹IO²ÎR?p^¨5J†?-¬Lkœ?p^¨5J†?ízݤ¾ïG?±ñÁCš?´)ٚ'G?±ñÁCš?횆 ‡?½'dö=£=?·[+͵ÁH?½'dö=£=?êaÇZÇ÷¦?°Ê…ªrH?Æxâ"à!h?°Ê…ªrH?ìæLwLh?žTcN?¸Í›'ûÂD?žTcNAGN4FGL J1728.5-7303?éÕ qMÀ4$ýó¶E¢À:Hä.bÀ<3+†–‡–@]îþOý@†Yùp™Æ?Ŧy{ìài?È5>eÁOì@Ü¢,æ@io‹þüJ?ïò';׿閗†™â•¿çÙ­…ߨr¿ìƒ[i³"¿ïͪB^Ia¿í³ð\ôÎAGNbcuPKS 1719-729?ïñÃ7ˆé"?^WAƒú?\yr{?^WAƒú?ïՄn)Ô?È?Tjħ?u=ÈÆÙqå?È?Tjħ?ïÊY'¨;s?o®SÂpÁ?zÓ>Œõʲ?o®SÂpÁ?ï°¦:‰5@?i0I&˜?ƒÖqjGü?i0I&˜?ïáÌu†aP?r±õzÿÇ>?n3Š4æ€l?r±õzÿÇ>?ïhê¿sjR?Ÿ&ìßÙó;?'â¨Jƒ´?Ÿ&ìßÙó;?îq'Cª"?žžÄ%×?¨í‹ÈÆcï?žžÄ%×?íK¢•ÁÅ?Ÿkq4˜?µ¢ëS<ìY?Ÿkq4˜AGN4FGL J1728.6-7448¿å
¯£ú¤)À4ó*®)s—À:ÄÎG÷–À<QiQ@Ã+Ìa˜@TÔ#&v?ʧ¹"ÓÝ?Û3ÿµ­K@LÛzåy@
¢¥Em(¿âîó2'#"¿Æþž–ƒ—¿åœ¼™xâj¿írJÀm˜à¿ïÿ—?LF*?à¯:ëŽYAGNbcuMRC 1722-748?ïäÂæo
?¨SÃE–`u?kñ<ôu-å?¨SÃE–`u?ïï1[l¸:?mX"Tãb?`Τ"GÅç?mX"Tãb?ï2	€9ÿ´?‡Ôß+NV]?™¾Ï÷;Œ?‡Ôß+NV]?ïô|ݲ^s?Boèdó?WDÚ{ê8?Boèdó?ïò0Ðò@?e],͊?[ž^EÏ ?e],͊?ï¶_ž(Ó?†çïål+?'~h
wK?†çïål+?ífWý€?§~³Y>?´ÍG×;-?§~³Y>?ï~5
÷?àä9¹<?9^Hõ70?àä9¹<AGN4FGL J1730.6+0024?Ì®ƒ>¿@2§Å¬À9;z6'À;¹ö&bjX@|ó€À¯³@«NoÑI?±Í .ɗ
?Âòø-}½@ìÂ
V)Ø@Ž»NöY?ï`8_¿¿ÕmÐ}†h¿â}»'!­Ð¿ã3øŠÀ¸Â¿ås•¹:¿ìEUt¦›
AGNfsrq3FGL J1730.5+0023PKS 1728+004?ïöKñ¿?Quˆ{ºº"?SéiÆÜ2œ?Quˆ{ºº"?ﱄ=֔?•üv¤RÇ?ƒžðšÙý?•üv¤RÇ?ï­¬ .ôŠ?'¾hځº®?""÷ôBÝu?'¾hځº®?ïü»WYƒ)?(7X2?:%C"ä†}?(7X2?ïèÌ9Kr'?bA¿=7ª?g3ÆuTžÈ?bA¿=7ª?î'r}Ôt¿?·Û…›Ï˜ž?­ˆØ&(P?·Û…›Ï˜ž?ï{Õg6V:?|"P€LÌ?…SVÙ?|"P€LÌ?ï÷ð-"ÐÇ?ALoç'](?P¤éöK?ALoç'](AGN4FGL J1730.6+3805?ïþ²Åå|ò@?ŠDØw$ûÀ;u¬Wâ?%À<Ìè^ùŠ›@!2ÂÄá
?ü `'çα?Ôy:éàÙÊ?Ó1¹KÈË?ü7«bï¹@´=«\9½?ڊ#¥ ¶Y¿•sÂ^M­¿Åûá¸AO¿ÚÒ²˝"¿ÞødÓiI¿ïÿîͨ"ßAGNbcuNVSS J173044+380452?ïøµda£?HþÃÔi­?M*mÚàPâ?HþÃÔi­?ïèójVœ*?mËÎNDð?g•´b•È?mËÎNDð?ïÁŸhvÈ?{"&
hòÕ?0Kâ(—
?{"&
hòÕ?ïÍÒxeö?[ eN}[?yvÉüQ
?[ eN}[?ï÷4¼——Ù?P"áH6Ôî?Q–†µSmí?P"áH6Ôî?ïµ&"gòò?ˆ­¦/ÃÖÉ?'¶^Ùü¡?ˆ­¦/ÃÖÉ?殺rgë;?†•Ìçl
Ú?†"ãsáI?†•Ìçl
Ú?ïVm•¸A-?'˜Kæ[\Ô?•2MH÷Ú[?'˜Kæ[\ÔAGN4FGL J1730.8+3715?ãrO™¬u%@?WðgȗÀ:NqªgG7À<ˆ}@@úÈi»°p?þ>ΌÀmC?Á×¢é¤sè?Ç=×&ñ@R4ebZh@)ߥ¥^?îìPá
¿æèm<C}-¿ÕÞ½ÛB[o¿àÞYçþ¿âš8%
|¿ïùK ½OVAGNbll3FGL J1730.6+3711GB6 J1730+3714?ïùŒ_Ê@?G‰—œv1p?KÅÎÅrÖ?G‰—œv1p?ïåàlfہ?pç/ýÞ7?j"³A†–?pç/ýÞ7?ïçjÁP(?fëi.
¢µ?h•>ŽÛ£s?fëi.
¢µ?ï´ÜfÙäô?`ƒ¿ë‡?'ÈæGÎôæ?`ƒ¿ë‡?ïòîŸZy?Yä³9ýù}?[Ø"•P®?Yä³9ýù}?ïµr''	?"=P¡bЭ?'£[Pgd?"=P¡bЭ?ïŽÔvºF?Žtì-h­Ž?ŒJâ[½0œ?Žtì-h­Ž?ï¢?ìH?'|ôwח?Ë¸•a?'|ôwחAGN4FGL J1731.6-3002?èyÈøú·?ÿ'¶@™MCÀ8èšÆÀCRÀ:ßPÃfò}@÷–ýˆ•@HËwb?·Õ÷ÃÆhÛ?ÆCž:h0Á@
uÐfµ@¿@1{ys‹¿ïþ}êªr?ïÿùJYQ¿Ü¶ûª¿ãA¾qg¿æsßVø¿ç£5ÄÝëAGNbll3FGL J1731.8-3001NVSS J173146-300309?ïÅýïÉ?é?''åx0¦?}oÏ^?''åx0¦?îšzfðÇJ?¨«Èm³ü?¦XY"‡@X?¨«Èm³ü?í1G:ª'?¦ZRU.ª?¶uÆ.¤¸o?¦ZRU.ª?ï,Kj h?€¿§ÿÇ£©?šv'½ä$ù?€¿§ÿÇ£©?îñšc1íR?¥d'éX? æYÌCå?¥d'éX?æ×w‰#Ÿ?ÎVü¢8¶?ÒQíý¸Â?ÎVü¢8¶?é×LÎËæ¯?°º<Ҙb?È¢ÌÄÐeD?°º<Ҙb?èóC×μ?¶4JoXá?Ì2ð Å?¶4JoXáAGN4FGL J1731.9-2719¿£7p'`֊@GëäÀ™À9-	¼AdNÀ:ßÀú)&@š¤Êû'@ØDŽŽoš?ÀÙÈ]ÒC.?¬øæÂR†œ?ñtŒINþk@{9ºHf?ïÿMB}þÞ¿ä/½BNF¿åA·ZtÀœ¿è,›Ÿ-WQ¿ç?B5.µö¿ÏDxjtèàAGNbcuNVSS J173149-271928?ïòžX£¸µ?a=©Åï?ZÃNÜJ…î?a=©Åï?ïTí¸Þ6	?£qƒúñ¯M?•bHìÐDÉ?£qƒúñ¯M?íäó!þ¶?¢ñ ÝþÊâ?°ØfðxCK?¢ñ ÝþÊâ?ïh÷ulé?zg…Z%p?'áUÒjR?zg…Z%p?ïÇt^?"'GS"µ?|xÅíÂ1/?"'GS"µ?ëÌåï2¨I?ğê»"F?ÀÌhC5^Ý?ğê»"F?í8|/?§©ÇØë?·–:gЌ?§©ÇØë?êëMàwh[?±€'¨zN?ÄRÈ~"^"?±€'¨zNAGN4FGL J1733.0-1305?ë{åäc–@%;À n À7†€Ǒ$À;
ì-4ì@õ ÿÿÕ@ُ¨?›dN^1ä?¿~™
,¹G@"? §?@žáW¿Á¥ˆço»¿àãÀ~౿äásLþ¶T¿ä.×N0¼¿ê:ó¼$ÞÝ¿ë.HG—nFAGNFSRQ3FGL J1733.0-1305PKS 1730-13?ïåúÚŒ'?fm0×y©-?j%Ýuîš?fm0×y©-?îD5#£HD?¼è£¢A‰?«¼­Ã7ÆÂ?¼è£¢A‰?ï`ʌšqu?'ÿó>[¶?"æ®niŸi?'ÿó>[¶?ïعS	­?l¶Ê˜ô9ð?s£V/ÜA'?l¶Ê˜ô9ð?ïxÒ¿fC?‡½‰-¨¿-?ü¡3ÿ§?‡½‰-¨¿-?étTŒZ}
?ÍgöÃZ!"?Ê.­Î–×?ÍgöÃZ!"?îüE4ßÓ?™'†Ñ——? ;¬´–"˜?™'†Ñ——?îµû3´Úµ?™A½BHØj?¤ LÇF	«?™A½BHØjAGN4FGL J1733.4-3943¿æ§ZìÀí·ä{õÀ9cßÏpÀ;oÅYa›@­T9éç@–-¹v®³?¹œRÜpÙ²?£dûØ(¯?êúâm©Q@p
xä¿å îؐO?ãæóŸI†Ý¿èä^ÿ"Ë)¿Úâ@|q뀿æ¤0ÌP¦¿×@êÁTs AGNbcu3FGL J1733.5-39412MASS J17332704-3942172?æ)ó‹[?ÝdÇK>Óá?Ó¬ÞéIÊ?ÝdÇK>Óá?ïÚØò±,?ƒa?r"†Ž³º=?ƒa?ïÉPݚ?Ò
ø¿Û?{y×겚Ø?Ò
ø¿Û?ïíÛK{å?N*vÄKLé?b$´};8<?N*vÄKLé?ïÍɝ {?'‹ËR‰Ç¸?y1qUšt?'‹ËR‰Ç¸?ï8E¾ûþ¿?«ÓŸ¢7Æí?˜÷H'_`%?«ÓŸ¢7Æí?ï\‡^í¯?•à·çí¢v?"o@ñæ!?•à·çí¢v?ïÿ°àï*?|bx´Bü?ˆ€Àäý"?|bx´BüAGN4FGL J1733.4+5428?ëÐZ—Á@@vÿCAž0À:"Ž÷À<m‰5žG~@MTùLˆ@å!ÂÈg?ËE'Á(?Õù"›…¬þ@ I@¼?øÜWYX6?ï,B³Ù¶À¿àáô±î$5¿ìÚ _†xU¿é¨¶7_޿á"Z¿ï÷ö'õ;AGNbll3FGL J1731.9+5428SDSS J173340.31+542636.9?ï—N¡×3?"(՘?«?Š>ì^ik?"(՘?«?è'Ioü?Æ°kfÅÉ?Í»²ÚC"?Æ°kfÅÉ?îÃÌ_l?šÕr¬¨'š?®3Ã?Ê	=?šÕr¬¨'š?çIKá³l\?²Fï^ºN?Ñmh<™'H?²Fï^ºN?íq¯µ·²?´mEŒRéo?´r‡ô
k?´mEŒRéo?Ë×ËËJ'?Ƀ¼ÇŠÝX?é

;
-v?Ƀ¼ÇŠÝX?ꘘÜ@™^?°[é‹6Žä?ŝœŽýš†?°[é‹6Žä?ÃGÁ;/g2?­¬³©o?ë.±4&4?­¬³©oMIXED4FGL J1733.6-6054¿ÉʞƒRJÀ-{¿PãGcÀ:÷8±!vÀ<0Ò­·]Ð@\U"°K@°h:{üÑ?¸ÐW›ÈH¿}Ëg<½/'?Âø4È4@+Y%¯g?B`Í ¿Û:"dKY¿äêkäT¨Ï¿âôšÜ¸o¿åLã=Qš'¿à•ªA°sAGNbcu3FGL J1733.8-6056PMN J1733-6055?ïþBt³tü?ïò+MN?+ظ|w±Ë?ïò+MN?ïõ
ü]^*?Yƒ­MChT?UêԐ|™?Yƒ­MChT?ïòÛ«H(õ?\JæTŸ?ZH¨ë½?\JæTŸ?ïþ>ulÏÈ?§!Uæ?,§L*?§!Uæ?ïüMÇÓÀ?4ÙdÉí?='Æ£x\?4ÙdÉí?ïÙתKm'?v^9þrÆû?s*ÑZ;8?v^9þrÆû?ïíîÖ¯?k?;j"gc?b*jðP?k?;j"gc?ïûx›6ª?2;Ö8(z^?B'1^ñ?2;Ö8(z^AGN4FGL J1734.0+0805?ïý-&Ì
@4Ü^³¾#À:{÷öFCÀ;ïÁ¸œ" @*¢Ø\¢î@'¤ŠŽd?ЕGûAT?ÝûÈ£GmR@·üƏ›ê@ç‰>W©Š?ï³Ä¾
'¿áî)°•	¿è
¼`îØ:¿ë\4-n¿ïÑÙ|¸[¿íññIƒ×AGNbcuNVSS J173400+080628?ïÁã;ñj2?"€6°¼?aè^jó?"€6°¼?èºùÚ2L??ǜ¾Ÿ	?Í—6Ï?ǜ¾Ÿ	?î,½¹‰y?œ šèï°?­?"'×j?œ šèï°?ë×|Œ?¢À€b`ÔH?Ã䢣¥Ñ?¢À€b`ÔH?íÏÄ/^+H?´ÂY‡Só|?±Þ†Æs»?´ÂY‡Só|?ÐsŸ"°PÀ?Ïkaüä?çÆ05§× ?Ïkaüä?ét°T'I'?²VÉ÷ً?Ê->­öÙø?²VÉ÷ً?ς¢«ª×ô?±ECœ†
?èWUJ?±ECœ†
MIXED4FGL J1734.3+3858?Ö¨횀R@?%á;ÛÀ8B9ҍ×À;¦ôlNô@`A–{@ÓÛÝr?òq»ÈÝC?µØçžp*@S,ü¸Lã@âà‹OÕ¿ÎAØi¿àW-^T¿äi\ð›Þî¿åÜ Ýp3¿ç½ŠÒS¿è§"ïQ0AGNfsrq3FGL J1734.3+3858B2 1732+38A?ïûu©qËA?@ûÍÚØH?B)Z.`ù?@ûÍÚØH?ïéÕzà	Ú?p|%ƒßÖd?f*…\oEt?p|%ƒßÖd?ïçû+ÚÏD?p´O©f»S?hÔ´/?p´O©f»S?ïÿ×ü?ŽX2õm?%#À¡:–?ŽX2õm?ïüYËßx1?7ꀆ2?=1Ÿ/Úo?7ꀆ2?ﺏäA¼?ˆ?S½\ ?\ôx'?ˆ?S½\ ?ïޕ	 º?}AR›Yhv?pµ{b"D?}AR›Yhv?ïý¦‰l$ì?,®˜Q%4E?2Ë´~õׁ?,®˜Q%4EAGN4FGL J1735.4-1118?Ðàø0†c@&p9ïôÀ:J­£;ÚÀ;Úv¾£>^@ µ[ÀE*@Cò%Kéã?ÂÍ1÷sê^?°
$àÎÑ#?ìÜ蹒]?ýiù¿Ê?âå=¿ë]ãà刅?³¹" k³¿à!ÑÁ©-5¿ä¾µÅ$b¿Ü|ö`D
vAGNbcu3FGL J1735.4-1118PMN J1735-1117?ïé'2á?b¥÷=ì!4?f}͵#éŒ?b¥÷=ì!4?ïv0ú&Ï?'HpìƒÏ?'9ග#?'HpìƒÏ?ï©5<*,?" ËʔÉ[?…²±eî?" ËʔÉ[?îƧÍË
¼?‡Ã4Z–¹?£•ƒ#OT@?‡Ã4Z–¹?ï­ª'IÐ?€®$9žóÓ?"•[ª_?€®$9žóÓ?ë½'{n?"Øqh'?Ác²G'?"Øqh'?ïUÅ{Â?–,Ÿ‹Å_?œ
õN/¿µ?–,Ÿ‹Å_?ë>·Ê ç[?¨A°~@?à Õ|b–?¨A°~@AGN4FGL J1735.8-5932?íLRÁv¸À,™¾ó'ªÀ:'çIOÕ*À<8pÇé8=@x/fŸò#@®œ£9UŒ?¿ZÝààô¿¢Ó›À\ÉQ?çGžÑÿ@a±"«É?ïòŒÝt¿éå»±–¿ê©bdy&¿Ò(>"$˜¿åuöâJ"¿Ý‡±d¼m.AGNbcuWISEA J173553.24-593204.6?ïù€Ü«´q?<v±G a?IüŒ€Ò»;?<v±G a?ïëò˜þ?nÞ+Íë¯?d
få!5d?nÞ+Íë¯?ïêÀåQ¯?`
Çä9¶¿?e?Àÿ?`
Çä9¶¿?ïó7̎Ó1?@QƚFG?YgEN]Å?@QƚFG?ï㙯A?f+íryš?lfçxÉ7;?f+íryš?ïÀ¥ûÉ?ˆæ"h`å¿?­|fçM?ˆæ"h`å¿?ï×Úâ^7?yLD`³ó?t÷à¨m?yLD`³ó?ï£éڂJ¦?t7³j?‡‰bÜòs?t7³jAGN4FGL J1736.0+2033?ïÙÂ¥Æ<@9kÿCAžÀ:yÇQcÀ<4¹º¡Q@`Ý•.?ûåå½^šÀ?»%33^&?Âڅ4-@	qá߃ˆ¶@L¯d‡/¿ÞTÕDj"?ïùînD˜¿Ñ0oço¿ÕÊÛ[	T¿áþàzÿzŸ¿ç#pvóÒAGNbll3FGL J1736.0+2033NVSS J173605+203301?ïýv:nç?05Å®žz?7ŒLM%³?05Å®žz?ïØQbž/Ö?ƒÛ[Ï r?s×N¥éTá?ƒÛ[Ï r?ïÛw\ØÉ?rëÄ[OŒ#?rDQŒYÕ?rëÄ[OŒ#?ïïÐP¡r?D;";¬}*?`/¯})#?D;";¬}*?ïôX©—ò?SyØbE2?WÉN{U¼@?SyØbE2?ïaóW"×?Ÿ¸±D­š]?"Á•#L½?Ÿ¸±D­š]?ï™ì׊?‰TR¨ôti?‰"Ê:Ý\Î?‰TR¨ôti?ïÓÃå%;×?f,hÐ6VY?v
Œþ|-?f,hÐ6VYAGN4FGL J1736.6+0628?ֵՙúÈ@3Ž7y…À9¢¼ƒ©mÀ;ÉÞuk¼ç@ÇÌIo4Á@ñ·?œÎ?¹gj3%?¢ähÂ-®Ü?áïk'–Fÿ@­éa'ý¿Ýê¬[¾Ñ¿å=yþHÅ¿êr(a&W¿âՌY?6w¿çiš-=Oí¿å‰á`ÈWAGNfsrq3FGL J1736.4+0634MG1 J173624+0632?ïõ™¶¹©É?Ph·Á·Ô?T̒µç½p?Ph·Á·Ô?ïÊIª˜ðQ?'\Ÿ¿Ø°v?zÛ*Ï·)?'\Ÿ¿Ø°v?ï¯Ù¥*úÞ?bÎ rÞ?"	–®º†?bÎ rÞ?ïÎþŸúÿ?`)VÛfr?x€°ox ?`)VÛfr?ïO.Ùxú?™—rÊc@5?–-ãÁ?™—rÊc@5?îÕn=³Œ?¨åÔ['•!?¢©~¸|:?¨åÔ['•!?î¤=_î
u?›-Ö¯{c?¥¼*ŽÄ¤?›-Ö¯{c?î´+½aä?'	´Ýãb ?¤½D)á¶û?'	´Ýãb AGN4FGL J1736.9-3357¿ï¯šP½¿ñ];_QŸ/À9"#æÀ:cçl‹C–@'.TQ;@̧…ëfì?ÒyÜ>YØ?НkJѵj@i"a9×?ùîþ"n¿Ê±,Þ/u¹?çepûì¿à¡ÙÙû‰y¿ç.Â5D0¿ëcoÁXûD¿ïÞÜÏyOwAGNbcuTXS 1733-339?Öe Œ'?ÒUªf›j?äÍw¯¹ìu?ÒUªf›j?ä=F|¼A?Îæ7LGI?ׅs‡Ù~?Îæ7LGI?á¼ò9Ì]?µŽŸ@"É?܆ŒgEÎ?µŽŸ@"É?åÔVDýÈ?³øV–Ï4½?ÔWSwæp?³øV–Ï4½?ÕD{)ÁðP?Ì{ˆ2OCÆ?å]ÂkØ?Ì{ˆ2OCÆ?ˤJS—?Î@*)@¸y?éík99?Î@*)@¸y?ØNe=Ç`Ò?·ì°Ù+sÚ?ãØÍaO—?·ì°Ù+sÚ?¸}úÃk?¬ûìW•?ìð@§ºï€?¬ûìW•MIXED4FGL J1738.0+8717?éÇ"A¯‰@;ô`RP/À:·9©MÀ<¯b³S@cÓù¼Äí@\Óû•74?À›íܼÙæ?¢ðæ t®l?âÍ*àÔ@´@Y‡2ŽÈ…¿î®kón!?ïý­_Ÿ!ï¿ç]à…ç5.¿ÜlOIoI¿äs¦¹Ù«¿â4¥>ŠFAGNbcu3FGL J1739.0+87166C B175708+871924?ïÿk#Ô4d?>¨{§¥?›V×eC?>¨{§¥?ï÷w¦¤^?SԞߝïž?QÒ4E¤ö?SԞߝïž?ïöå·Kӊ?TE'¶ž?R4'éŠ:\?TE'¶ž?ïÿì¶eñæ>Ôüv¯Ý>ãIz¸l>>Ôüv¯Ý?ïÿdHBÓ©?ªC±9?vðÒ2Øu?ªC±9?ïÜFñ£?xÒ(½°W?qö÷ZwjO?xÒ(½°W?ïøNÝU(?atʪÐ"?O'âll?atʪÐ"?ïÿå¶Ü(=>ëVYI`Â>êHòOPOë>ëVYI`ÂAGN4FGL J1738.0+0236¿¢o˜‹žü|@1€*ýڋÒÀ:n@÷À;ÙYæ%cg@´Þ'›¦@ÚÁLf
 ?ÍùdÅÒ\¯?¾$jÃmR"?åü§…ëg@#+©&?éVˁ¿ØÀPýôb¿ì¥Ž¿öЁ¿íÒÅ4R$?Ð웟-WQ¿¢HtñoÄAGNbcuPKS 1735+026?ï×8îÞðf?6@;«é?tcˆ•WA
?6@;«é?0½äì?	ÝÒÛ9?€ÛÐ}ç,?	ÝÒÛ9?îñõ¨R?•ýÆP*Ð? î¢C…?•ýÆP*Ð?ïø¿|à®à?>¬îÀÿmk?M
¦DL?>¬îÀÿmk?í#©tÐXë?¼—Üø`pÐ?¶â´[¢ú'?¼—Üø`pÐ?íÑæ9–‹?¸ª˜n.-{?±wÀÎ3K©?¸ª˜n.-{?ëð(üšè?­<'"¿­?À?\
"_•?­<'"¿­?ᅱ?‰I¾q«Õ?Ø"Ë«k?‰I¾q«ÕAGN4FGL J1738.2+4000¿êµUg:¡¼@>z'ÓºþÀ;ƒšSÓ½À<7‹öBçÜ@QÎCÅQ®@©ÚßµÝ?Œ)™pÙ¿µH@Ô±s?ò¿zÊÒ!@¦%‹ªÃŽ?ïÌi?‰­¾¿êúcÿÿå¿áŽá¿Î¼¿êqH'Š¿¦I`àÚ9·¿ïþâ=ø3-AGNbcuNVSS J173807+400312?ïýêðù?,R»ŒÊR¾?0¨«ê_?,R»ŒÊR¾?ïòb`ÐØÔ?_žæWê=?[;>E'(å?_žæWê=?ïéD4jã?kh¶'?f»â
ÍìŽ?kh¶'?ïý{,¥?(ܵÄÎæ?7ä&ŸjØ«?(ܵÄÎæ?ïû¡Æ—\?C¡ÎšéO|?C¹y|Ñ^m?C¡ÎšéO|?ïÇÌ9ÿÖ?~C»>£Šy?|ââˆTß?~C»>£Šy?ïÛãÎú'?tÑÒ·X¤?rv`Zç?tÑÒ·X¤?ïáaYaE??j·•µ‹Ëü?nž¦r¿Àî?j·•µ‹ËüAGN4FGL J1738.3+3228?í%êÙ¹Uˆ@<´›ùÆ*À;8Áo¡x‹À<}uôxãA@қ&·yÔ@Ÿ¾ÿ"°?Áø¹ò8¿»ˆÖ}АQ?øÅ̒ë)¯@ì|a$ˆ ¿êÓB1Ó¸¿ä̹ìö8¿étyN w¿Í{«ÝhüC¿ïÿÿ&¦³?ïÿûÞ]BüAGNfsrqMG2 J173841+3224?ïúøg…J?RňžÁ??Gèt›é¼?RňžÁ??ïï+è¢QŠ?fãŽ{zn?`ÔaÍý³?fãŽ{zn?ﵞƻL?"—$r›Àö?'˜NB·Ž?"—$r›Àö?ïü@vxé\?0Ú-vÉÝ?=üL€,ÿF?0Ú-vÉÝ?ïî<] ¼p?gŒÜÏPÄ?aâ&éøN?gŒÜÏPÄ?ï¶Ï¢¥r?‡‰%ôp?'LqŽ?‡‰%ôp?ïÅé ºlš?ƒ!ýWŽo?}/­ÈrÇ?ƒ!ýWŽo?ïÇ[ñîDl?v7…PU?|R恲P?v7…PUAGN4FGL J1738.8+3822?çÌÇޝÒ@>ȸkùÀ;îQ{‡À<ö¦€1ê@!ØÚøºº?üóìFØ
?ÔrIÞñ<™?°å#/Úä?Ù[^€=ýç?ô'=ìs±?îÝ\á0¿ïE¸põ5¢?Ö ÎAAð¿é{S]u&¿œÊîÙŌD¿Ç-q}EÐðAGNbcuNVSS J173842+382104?ïÈav?o?´)ú;Óæ?{Ï1SN¤…?´)ú;Óæ?ï蜪"ÜW?ft€œ#âà?gcUÙ!{?ft€œ#âà?ïÀ¸š6´?\Àû/?£ôErŠ?\Àû/?ïÚwÁhÑ·?`rqÛ9J?rÄ+JÐÄ?`rqÛ9J?ïü‡Ì"éö??°žÁãd2?;Ášåb??°žÁãd2?NœÞ?œ–šwR€?ŽÕlbçœU?œ–šwR€?ï´ Où	
?†pâ—ïˆT?'÷ìí¨?†pâ—ïˆT?ï}®ùÊ?"/*χHP?œDù\·?"/*χHPAGN4FGL J1738.8-3418¿îZlDn;i¿ùצ•*ŸÀ9O¡(TÀ:zòl™†N@ã""i·T@`ô¼ÕÞÄ?ÑÚ£Š´$?ѵ<O|@>EedÞ§@Õm¸?L¿æ"PA`ó`?ï%…€]˜¿é#Ê?SÒæ¿çb_I¿î'þ¢‡ÔË?©wìÎQ‡AGNbcuNVSS J173913-341749?á­ëMk?Òæ3¨?Ü¥éÄ)e)?Òæ3¨?é|
oTK²?ÇÙøRü@?ÊÊB®Ñ9?ÇÙøRü@?äĵ	?Lz?·E¢¡Å(?Öv•íg
?·E¢¡Å(?ë…+0—?«ŒV
ß¾'?ÁëS?î¦?«ŒV
ß¾'?á{ÇîãðL?ÐSOƚ?Ýp"8g?ÐSOƚ?ÙñJq#"ì?Ô´À/Ê6ß?ãZÇn5Š?Ô´À/Ê6ß?×1:.
f?¼0,˜Xx?äg@bèúÍ?¼0,˜Xx?È#w¾Ódì?¸"ÿ/ÝK?é÷"K&Å?¸"ÿ/ÝKMIXED4FGL J1739.5+4955?²Üæ/w+@?·¸€®À92`8NûçÀ<CÄzî´@!;`©8@)æ~Nº?§ûîxn%Í?µ¸¡ÄË@
_`ûÃZ]@ã¤bËQM?ú+ª©¿á^Z(j'U¿ä¬…>õ!¿çêÿè­ÿ¿å•‡9᣿åE~Y¢2ÅAGNfsrq3FGL J1739.4+4955S4 1738+49?ïÕBþ"Š?¢Œœv'Ùf?u^€´àbÒ?¢Œœv'Ùf?ïõO¯¸l?Yzõ×?'ð?U` Ï!÷†?Yzõ×?'ð?ïà*f…ñ?w}4ãµ
?oùÕԓV¾?w}4ãµ
?ïý«ß8ׄ?!6@Z3N?2¡j^æ'?!6@Z3N?ïþG‹¯Ì?"wsâ:
?+‡H_¾+?"wsâ:
?ïÌ´gatJ?"ææf)k?y¥ÌpBŸ?"ææf)k?ï«ïðÆÚ£?"§«›õÍ?…Ѹó;?"§«›õÍ?ïú÷çq'"?4ˆÒ1í|?D bÓWvD?4ˆÒ1í|AGN4FGL J1740.0+4737?×íÈ^ÂÇÕ@?_Ãb(À:< Ÿ²¸OÀ<aë­b¤@¾éõ§Œv@$§š
\à?¼åúÆ/O?±."AS?õÔpšœÎØ@©Ì?ïÿÍ_ï©Ç¿æX}o—h¿ã1Ÿ_VQÆ¿Ùº-Ç©­¿ãQ@¾Œ¿æä&ó|AGNfsrq3FGL J1740.3+4736S4 1738+47?ïþMø''?"‹:½?+'™c£?"‹:½?ïójê?à|?YO.ŠÛ§b?Y*+Í6GÆ?YO.ŠÛ§b?ïøÌD:?>¹¿;?LÎï\Í,}?>¹¿;?ïê¢JÃË?H§á1òÁà?e]µqDü?H§á1òÁà?ïþ¥ºÜ'?&<Èl?.e¦ðë -?&<Èl?ïÓ¸,'ì=?x_o$›­Õ?v#é¡ì9Õ?x_o$›­Õ?ï÷fdŸ"+?_¥^åæ¾®?Q37ó9Ü?_¥^åæ¾®?ïŲŸ­u?d/äXŒÄ?}&°"Z
Œ?d/äXŒÄAGN4FGL J1740.5+5211¿àÁŸ2=r…@?ÂU:Ä÷ìÀ8'Û¼SØÅÀ<#ÞËÒÒ@Eãdú@œ¦Êı?[œ"?¡ñ=;í
?ü.x?'æ@¹'ÇÅüϿϵšðg¿ãõ"!	ºê¿ç?']<9¿æm7:ÿ°¿åWZà f¨¿ê¡7¦®AGNfsrq3FGL J1740.3+52114C +51.37?ïþ̇¾¶ñ?IkM:—?#7…%>ÀÇ?IkM:—?ïõýõ'£¢?Wè¤m¬Ü?T'|,–?Wè¤m¬Ü?ïíhžO?nÀYÝþÀ?b—a¤–h?nÀYÝþÀ?ïÿÕë%õª>ðÍ WX>õ
Jñ3ÂÛ>ðÍ WX?ïþã´+&†?
ÿ?õ‰?!ÄÀ̘HÌ?
ÿ?õ‰?ïؐϽåK?w俖..?s·˜.Ëʍ?w俖..?ïèËÀÖ?qW¦~ˆ1ï?gré.¿Ês?qW¦~ˆ1ï?ïÿÙâ_I>ïßÖü\â>óÁÊcœ>ïßÖü\âAGN4FGL J1740.6+5346?îÙdý"@?Úuy(àÊÀ:WÑù\xÀ<zp§@Xâ»Ìtb@ÀàpÀ?»Æ.£ ?½…®À>•@ÀÄù™´r@oo.ah¿áDãß»¿æ\ÄÞÁ¿âVÂïÔ8Ò¿àîÚÞÞGI¿â	w­¶‡¿êÕC^#¡ÆAGNbll3FGL J1740.4+534787GB 173932.3+534742?ïþZh×.û?A^¬Öè'?*YpH…§?A^¬Öè'?ïô©é%¦‹?X¯>Â>› ?V¬-ü*É?X¯>Â>› ?ï÷àëMýu?b¶{ÂMØ?P>)Ô+ˆ_?b¶{ÂMØ?ïöÁ	õø?6ù|j¼C?R}ì	s?6ù|j¼C?ïý2'ø?22Cq?7^iØPDõ?22Cq?ïТ±è'H?€rkÒüx?w®§#4?€rkÒüx?ïúÜfº?UX¬	úÒß?G€ŽÅs<?UX¬	úÒß?ïÚÙõ
?`["ÚŸ¡?r"r'ٍü?`["ÚŸ¡AGN4FGL J1741.1+7226¿íýO&"@?
¹pޏÀ;	³Ýè~À<ÂDK‰kN@:äƒøž@êp?ň.!Ña?¢¬Okx?Ü[Á|Œ˜?ùšw_²íþ?ìµæSҐ¿Ü¼ã`7"V¿æÃr ÜY¿äAß¾–ÿ¿áP2芘u¿ïÿX¥³ƒPAGNbllGB6 J1741+7224?ïû^
æþ?8ãUd£Ã'?C¾‡Š¹6â?8ãUd£Ã'?ïä)·Ö½ß?r~u}(?kÖH%"™F?r~u}(?ïҏƒZì?slÈz_œ
?v¸>0£r?slÈz_œ
?ï©á2èé?h}Ž1uð?…‡³;væ¡?h}Ž1uð?ïõ*^Þ?OúšQÛ­ü?U«CÜÁì?OúšQÛ­ü?ïi"æ¯!?œ9<˜©Ýô?'Ïc&¬A[?œ9<˜©Ýô?ï+žX4
?†V¦xüËU?ˆµ{!Ž?†V¦xüËU?íÙQ9p?—~ö\—À?±5v6@˜q?—~ö\—ÀAGN4FGL J1741.2+5739¿Ø÷"ÁME@?븝jßÀ;ø¢t4À<­2.@ö睸0@eÄ÷1$?Á"ÑöØ9¿¨Í¼ì"ù?è›NÇ@
JML¹ìö¿Ø…o«‰†&¿è"Lá<P¿èbs'ƒ¨l¿à"NÿA"¿à*6¡Ó¿â÷,ò§QéAGNbllNVSS J174111+573812?ïÿ&k¤"É?
í©Ñè<?2'©Èt?
í©Ñè<?ïöÛÜ<à?U°µµ‹=?SÈHJEð6?U°µµ‹=?ïø¾y??S‹ZáRãÎ?Müßì£?S‹ZáRãÎ?ïþsº{«6?âŸðй?(ÄZŽ=Q‡?âŸðй?ïÿ$eü¸?Æ¥BM܈?sFOw?Æ¥BM܈?ï×þºì¶³?w.d̛?/?t¢z†^t?w.d̛?/?ïùsL¹þ$?TØón®Å?J2Í:b!?TØón®Å?ïökqàd?Eç&«¸½³?Rý)7¼ã?Eç&«¸½³AGN4FGL J1741.5-3119?鏿åw'\¿à¾+IÀ9CUÚýçøÀ:Äz³ûD¯@È©¿±V@t6¸ù±1?ËϦ›à›·?àÜ{@" @¤˜"¡¸?ü(3/­AÂ?è<ÉIŠ¿è°«#.Ù¿ÐÄ?Êñ*z¿ásÇ­©¿ìzׁ܎Œ¿îpÍÝîÞAGNbcuNVSS J174126-312329?Ñ4p;ý1?É¢1|2ù?çeûÇâg?É¢1|2ù?ÖjJ¾Œ'?ʹ3?	o?äÊÚ ¹¸7?ʹ3?	o?ÝV:qÆ}?³ëfÙÃ?áTâðGÁ?³ëfÙÃ?Þi«îc~?³…$vê´?àË*Î@ü?³…$vê´?Ï9ýçeÄ?Ët1¨øø?è1º†&?Ët1¨øø?£^؂¬zï?³7@æ:Œ7?îÊwž>'?³7@æ:Œ7?ÀrÍT(˜?­·²;)‹e?ëãLªõÙÙ?­·²;)‹e?¨7`ìd?–ÚØB´?î܊¼Z?–ÚØB´PSR4FGL J1741.8-2537¿ç;£u¡¨î@¢å€!ùOÀ8Ôê~ŽÀ:æ[{PÙ6@ &½´«î±@'ÞkZÂ?µqÞ>º$ÿ?Ûä'Z?ÜW!O Ñ@tKøÑãb?íø©)Y•ž?ëù>Dß-"¿ä΢o>¿ä8kì¸$Ÿ¿à½!Þ÷ò•¿äˆ×~×AGNbcu3FGL J1741.9-2539NVSS J174154-253743?ïÆ×)òíž?û
¨F?|"kG¡?û
¨F?ï2åþL À?©·¦ö©‰	?™£@9ëƒþ?©·¦ö©‰	?í.ºnŒ‹Ð?¦µxDи–?¶Š,Š¿º?¦µxDи–?îççXFñŠ?ŒºÐůæ?¡Š~$œb?ŒºÐůæ?í³ÆѲ)?µÂ\`;?²aÉx`b6?µÂ\`;?êu;žf²ç?É®\‰Ã¸§?Æ+†e4b?É®\‰Ã¸§?왶YÆ2?­Áǂ's/?»2M7ÉÎs?­Áǂ's/?ëÀItpÈÉ?°ªj5ù˜$?ÀþÚ.<ÜÞ?°ªj5ù˜$AGN4FGL J1741.9+2555?ïí²Ž:É]@9ý•1ã¨À;,PFipÝÀ<­^éšbí@½!ØAõï?ï0]€c½•?ø£Ðä¿?é¾ý×0ÓÝ?ût8Ùeb@-bŽÀx¿ê×ëC°Xù?ïÉxQ{¿å4µê28¿¡ý Ãô$ï¿ïÿú Âî'?ïÃk$;H«AGNbcuNVSS J174147+255443?îñ¥ EÛ?¾Î	Ҁ"¹? å®Å»N?¾Î	Ҁ"¹?ï›Ì;*V?¢­,†"?‰üô¥t?¢­,†"?í

:†?¢'A÷ÀB/?·¯—4tÙ?¢'A÷ÀB/?ï¢òÕf­?z3‹‰¿¾"?‡CJ»6¸©?z3‹‰¿¾"?îᐮŽsK?¨¦ÐÏ:æ0?¡æõЙQ?¨¦ÐÏ:æ0?î`'2Añ'?½ö®G¦‡¿?©öìÚ)ã?½ö®G¦‡¿?í~íKÐìu?¢rkQcž+?´•ŸRÚÝ?¢rkQcž+?ï)¼ÿì#?"oÒ=''f?šÈ~᳞?"oÒ=''fAGN4FGL J1742.4-1518?Òèô
Œ
H@פ?åÉÀ9Àºª‹YeÀ;_Œ™¦@*ò03¤r@1ú´f¤?Ðç=¼h?݆T"A'@~€8Ÿ"@¥uT ?ïÿÉ仿⸗ÁREG¿æ×í\M¿íø < ¿à— /µÐ1¿îôú¬)AGNbcuPMN J1742-1517?ï@€JÊ?£E×óJ?—ïö¿ÜÆ·?£E×óJ?ç¡0ð@wó?Ȕ¼|¿æ'?нž?Ȕ¼|¿æ'?ë´¤ºŽ¾?¨âªOav™?Á-mýÅ
?¨âªOav™?ì BV1?¡]˜}ãü+?¾ýì-Nu?¡]˜}ãü+?í=îû­¶?·²v_WÔ?¶îØ·Ó?·²v_WÔ?¿ñ}þïœ?ľö*>B?ìÐ@0
?ľö*>B?âôˆldq?½ßÍ×a?ÛÚï'7?½ßÍ×a?Ö"Cqò?½ƒ>R9øc?äü½ÞGs‡?½ƒ>R9øcMIXED4FGL J1742.5+5944?ìFj­m@?Ⱦ
í(À:(1ø .À<˜Â^§U@';‡j—ù@RI^ãL?¶WfwÆ?›šà|¾'Õ?å‰Eû7@·º×Véq?îú¨Ü,¼¿åÒÑß^¿äø!å-¿ßÈh"M×ú¿äpƒڐۿäÍÝ·×AGNbll3FGL J1742.2+5947RGB J1742+597?ïýÂx‹%?"Jˬ\æ?1ì<pF¦?"Jˬ\æ?ïõ/&´Ö?[	¿é%ÿ?U¡²»~CÆ?[	¿é%ÿ?ïùþ›?SŒ&6óùŒ?I‹ÜZÉü?SŒ&6óùŒ?ïç°Rîj?Qs7è1+?hO­1ý"?Qs7è1+?ïûøg
?4»P£C?@cfÐÈ?4»P£C?ïÕ¾2«#?zéòq©êå?u æQv1?zéòq©êå?ïû/èRÖ?OؔAÏå¯?C@`7Ü\"?OؔAÏå¯?ï½±j+þó?iÿ{ZED#?€"¥ywÁR?iÿ{ZED#AGN4FGL J1743.9-1824¿êäò»ý@5JœÀ:%N1¼:®À;欇²çH@íwÜ°oŸ@Ýœ®÷Ð?Ð3rôb³?îhOt²Y"@èK èBt?÷1=ª…z(?î»ïÐð¿ç±aË×Ú¿ÔÂ܉r¡¿ëDjÞEE/¿ïÿßéà
¿êÖj€˜AAGNbcuPMN J1743-1828?Ÿe?ù(ñ?§'ZmÐ6?ï"ÕÖûi?§'ZmÐ6?§Búú¨??¬w8uÜ2î?î‡+Ð4؜?¬w8uÜ2î?Ó AQa¥?°ëLA[›Û?æ/ßWO-v?°ëLA[›Û?JÆ›Ô?sžÄ&7-³?ï}©Îðéb?sžÄ&7-³?f?^´WÁ?n'óÈã«Û?ïéÀî, ?n'óÈã«Û?x´ldrgq?‰SF‹ñ˜?ïΗ'Nx‰?‰SF‹ñ˜?³í¤$ÊI?£GÏ>Åw>?í'Kl÷?£GÏ>Åw>?Auˆƒùʉ?1àf©†S?ïû¢Ï3Y?1àf©†SPSR4FGL J1743.9+3747?î$5úÈD@<è˜_ö"À;g5¼zo2À<»-0º²ï@g³îY?ÿuÖ[æ?çéR©ðÿ²?Ø*HþÌy@?ógÄՇ†r@œ*M[}¿ïñ4 ›–t?ïýìo¡Î¿ß¸7^»ø¿àͶ!Ãg¿ïIűO˜Å?ˆ`NQû(AGNfsrqB3 1742+378?ïÅ Ôi×?ì6õ_"?}o•Ö=Ô??ì6õ_"?ï꼿c'±?i¨µ ?eC@–ýî½?i¨µ ?îñ>E­U±?Že¤wÉ? ì¢–ïû?Že¤wÉ?ïÕ9ŽA!?^<Y`85ç?uwc?»‰?^<Y`85ç?ï»R§þÈ?"Ÿ6ä$l?9+Yóæ?"Ÿ6ä$l?ïªO¢«?Œ:ÔJ:?…l 4qÂ?Œ:ÔJ:?í´a|ØÔÔ?¡Qò)íS?²\ôƒ3Þ?¡Qò)íS?ïJytF_?…Çg´-?–°Ñxëê˜?…Çg´-AGN4FGL J1744.0+1935?ïºß'³@7SÒǸÖÀ9rƒ\@sÀ<ÀÑìÇ>@¼ß7Þh¬?þ"à¿ÈØL?±'×
hcÂ?¢ûW¾q¯	?óÄÞ ²'/@‰Î³£?ïÿÕØå	¿ÂMæ<à[¿áìÙ|Þwð¿Õ³~G-»û¿â›õ>…÷¦¿×»s^"0AGNbll3FGL J1743.9+1934S3 1741+19?ïúÿG'?7¦¤¦0"?D‡i3.º?7¦¤¦0"?ïÜP—v¹?v€(ØÞøL?q×´"óïw?v€(ØÞøL?ï誮c?hÀƒwº?gUR,ö•·?hÀƒwº?ïš'W«ì?qó²ÑæG‹?‰v?4cØï?qó²ÑæG‹?ïô:ʁC?Sá·m§'Â?WŠk
ø¸?Sá·m§'Â?ïoüÝ? ~ô¹V?'|˜%'? ~ô¹V?ïÔ©S0÷?|Æy©6?u«wGù(¡?|Æy©6?î÷wò;,?‹ß‹áãð? ˆ€Ù¹'3?‹ß‹áãðAGN4FGL J1744.2-0353¿í5¡ä…"ï@*B®Ñ9CÀ9Í·'Ò$ûÀ;…}Ý{pº@ÕpK¯@meie?Öø]i?³ás¢äñÝ?î=Å}£ô@+NVÀ¿ÕpÔ^;Ÿ"¿ã
8bGõ¿è4Ž}å¿ä˜òü¿èÙïÊþ–¿ÂÒ°X¢AGNfsrq3FGL J1744.3-0353PKS 1741-03?ïüm`¢úc?3¤´[Þ6ž?<"øãg¬)?3¤´[Þ6ž?ïº×:t?ŠéaÌÜc¯?J8&Üã?ŠéaÌÜc¯?ïß	taÀ~?p7o|Àh?p{E×^Ðã?p7o|Àh?ïê>Ý,ã°?J½NãK#±?eÁ#Ïo?J½NãK#±?ï÷¥w¨½?K®6'Ž¸?PµÔò•É?K®6'Ž¸?î8¸oêëé?µwYë¾0{?¬tyÀÝj?µwYë¾0{?ïhtí	Ñ?%n²6ßÀ?'ñ}Ä"í?%n²6ßÀ?ïOTîç X?'¸ÛS¥Oú?–bô‹?'¸ÛS¥OúAGN4FGL J1744.4+1851?åm¿²CE@6ø/@_k À;\ŒñšÀ<™ªæÈ÷U@!v<_+߂?ü²7Pþ?ÏyïÓ»©?ªl…©?܌xžÍ5'@"`PÍ¢á?ïée߭п형";"+¿Ø¥þ—J4¿¸þ2ËYZ9¿çàm"R¿»ÉÐn
AGNbll1RXS J174420.1+185215?ïþrC¿G~?!t@æàǶ?(ÛÁ@ÙbR?!t@æàǶ?ïã8𝝛?}i…úRw?lÇV̤?}i…úRw?ïAå(?dfjÊU??aYC`(‰?dfjÊU??ïòc¹|§µ?Cµ#²]À?[8o$µ?Cµ#²]À?ïþ"E‡m?"\øb›?&˯˜$†O?"\øb›?ïz5_L/?¢3àŽOØ?¹TšÔa?¢3àŽOØ?ïäé¥XG?u=éMO?kô#­ù?u=éMO?ïÕ,þÌàT?fæè§RÑ?ui€‰¶?fæè§RÑAGN4FGL J1744.6-5713¿äsÿðÕYÀ,\8Ÿƒ¾fÀ:
ٖߪöÀ<L|f'ëØ@ DÁ^.´s?þњw+?¼¯éè ?±tÏ	èâ?õ­`öºÜà@xM"µm?ïÿþÞ÷¿æ´ÇóI8X¿áX(`s¤¿ÕÙjj%š¿ßWÛßm׿ää2pLAGNbllPMN J1744-5715?ïÿÀ·žE?䷍™O?g繑¶?䷍™O?ïó$=³%?dâ
s'ŒX?Y·"÷+1:?dâ
s'ŒX?ïõßzEã±?c›´tS?TAŠ6?c›´tS?ïýEyöè?–Û_,Š?5Ô0nv‡?–Û_,Š?ïÿ뇼¼?'Ú¥'?'—	å×?'Ú¥'?ïÊpJ¯•s?–›Xü×Ñ?zÇڅÙ.–?–›Xü×Ñ?ïù=©-á:?UXØ(¶… ?K	[šdû¼?UXØ(¶… ?ïù°x-c;?6ëôªätF?I>re@'?6ëôªätFAGN4FGL J1744.9-1727¿îFºÍ×õÜ@`\÷QÜÀ8ÁD× eÀ;… Äe@ ´©‰¦²\?þú¿"íÚ?ªŒŒk‰?'Ò1n?¬F?Øvd4¾@"8­ñjf?ïò6ci\¿Ü,ûáN2¿äJ¢»Jî¿×a¿â;˜ý'gv¿Å!("-¡¤AGNbcu3FGL J1744.9-17251RXS J174459.5-172640?ï÷jãðø?Mz—Œ?Pá*£°?Mz—Œ?ïè)ìÚ×? /"ý"xì?Œõˆ8æT? /"ý"xì?L•¸l?ŽyŸ '&ü?'ì×"Hý?ŽyŸ '&ü?ïƒÓá¶`F?4NZÎ$?™G&j?4NZÎ$?ïم¦¤Î?rOÎVšU?s=9PA\?rOÎVšU?ìŠQbHI›?ÅC–"Þ˜ô?»­tí½³)?ÅC–"Þ˜ô?ïH>9Ä·?–¤Säõ?–ø?:7+?–¤Säõ?îÙ¡–Š'ã?•þ+aÏ?¢e曢TÌ?•þ+aÏAGN4FGL J1745.1+4731?Ù‰uÏ@>ƒô˜Ã°ÄÀ;T֍?ïÀ<¯l‹C•@º
.k?ýñ%Vѝí?âN.r±M?ÖÄ2I~?ù[4Ú@vkÿØgá?žÖ=
ýn«?ïÿnw¬à¿äY®'3÷S¿Ùv™ºPÉF¿é¢·…<ëC¿ïÿð ¼x—AGNbcu3FGL J1745.4+4721NVSS J174501+473247?ïô×ô¯P ?a	ÿ¬©®?VP3l?Ï?a	ÿ¬©®?ïï
Žç0?`Ð 
Ï&?`õ÷€7x?`Ð 
Ï&?ïiª·ŠV—?‹×~š"(?'Ê©µ-'?‹×~š"(?ïڔZ.c"?V"@É#f?rµÒé~)Ã?V"@É#f?ïñh¼,?bkòv
{#?]É.uE??bkòv
{#?ïÂÄX½Žõ?'Û;}?(?~Ó‹êñ±?'Û;}?(?ï='
Dr\?'¹-,'?˜M¾ZáP|?'¹-,'?Œ¿Ã?~sãLw@?V\÷às^?~sãLw@AGN4FGL J1745.4-0753?è¹Cá‰Ð×@%£ôË—¦À8ØûíKÈUÀ;ktà |@Ðrá@‰å\ËO?ªŠq¼
•r?†:¯1ƒ?Üùº@®@øìÂ
¦ø?îÃpbhªä?á¨Ü,¼!¿ß¢Ž4ቿâòMà]£I¿áP©ôg¿Î'ÕDÀyWAGNbll3FGL J1745.4-0754TXS 1742-078?ïãgFyü?c'»
_œ?l÷˜Ù"l!?c'»
_œ?ïzÇ&D¸A?¡ØêÑëQ?§:ؓá?¡ØêÑëQ?îè!­Wo0?˜žüZ+¯?¡}å-Áø?˜žüZ+¯?îy«ÌÖ–?—Ó¿ÿ4?¨eC4^á ?—Ó¿ÿ4?ï#Ø8¡î?'¾|yŽ'r?›÷3ô;?'¾|yŽ'r?íIçVTº0?ºVê¦??µ°ÅOü{?ºVê¦??îÒõÏê'j?œ³:vë¼?¢Ð¢þÉÔ]?œ³:vë¼?ëâ™ç?²¶RL~î?Àw—јc?²¶RL~îAGN4FGL J1745.6+3950¿ígO¼Î@=Â!yÀ:ôÿ—$tÀ<¢þ~ö€$@Ú%Oð®@ËÛjõA?ÀTUØ#Âþ¿§ñi~º?é{~h?ý‰J°Rn¿ß?ÒéF€¿æ›#Â|粿àÉÍ©kžµ¿æ[Ù_'F—¿ÔöÜÀµ½¿Øˆ]|\òÊAGNbll3FGL J1745.7+3952B2 1743+39C?ïúõ(­ëƒ?5ÙY\/ù­?D+]Â]®©?5ÙY\/ù­?ïî˜}KŽ?aÕzNZk?ag'¿é1®?aÕzNZk?ïêÿnEê?c32bJôU?e'~ü¸?c32bJôU?ïëÆû;?K ˜p0=?d9é(¢´i?K ˜p0=?ïçs<kH×?c­¥ÍÖùQ?hŒÃ­tX÷?c­¥ÍÖùQ?ï±÷Thk?…í¡A`R?ƒ¿Â$­_?…í¡A`R?ïäïPQÉ?toBšaô?k~oŽì?toBšaô?ïNEKÓW?†<Ò2+:/?–-÷]dÍ?†<Ò2+:/AGN4FGL J1746.8-5235?î€
I¸ŽÀ(v³™õßìÀ9Ågqÿ ÝÀ;ª'°H1È@^+?ô·¢@VF]²c?½—Ù%Ê ?Ï¡G"~Z#@ÔnYyîÙ@Œ>gCÜ?îÞé?Mô¿á]ʶr¿åî€F}¿æI'*K'¿î…ýÉÄÛ¿ïýß1S_AGNbcuPMN J1747-5236?ï§æoÏàl?†ßH Ø?†dw€æ?†ßH Ø?ï踏—ÑÝ?€8áu¶Èw?gGp_ïð?€8áu¶Èw?﻽A$Ê?Û±Ð?ŸˆˆR³üÓ?Û±Ð?ïüd$AÓµ?(!kÏþm?<ÞÞ]"äœ?(!kÏþm?ï¢ÜI¨§?"'ü?	Ú?œK¤}ª#?"'ü?	Ú?ï•ê,PY?žÿt=4V?Š…tèm
á?žÿt=4V?êkø²¿ì{?¬t5øX˜}?ÆP5N?¬t5øX˜}?ïí¢k
$?Tp¶˜ Qh?b]"å8¬)?Tp¶˜ QhAGN4FGL J1747.1-5453¿Æ™0ŽÏLjÀ*Àaé)#æÀ:=ÀÙyƒzÀ<	¶Å#‹ @Ä>tÎ@²ÔüF7?½g'¬lZ¿ãKX1ß?Î]èHSV@'ß–S"?ïøæ0K!g¿äFÏAò׿èèmÀÍ»¿âMrU€¿ä…áUðÍ¿éï¯OäCâAGNbcuPMN J1747-5450?ïþ'VõÉà?"j`âñj?-Š(<Î?"j`âñj?ïóñš?9"?\æ"æQ?XË`·f?\æ"æQ?ïò¨˜Sã?`QÞ6"Ì?Z®ÏBŠ³?`QÞ6"Ì?ïþÈFø"X?
½}·HT5?#{"K5+?
½}·HT5?ïýûµ\\'?&¡Èª¤!?0"V° È`?&¡Èª¤!?ïؑ줌?yBº-S?s·v&ŠqË?yBº-S?ïéÐhý^?o'«Vmf?f~/c¹¹?o'«Vmf?ïû¹…ƒsN?22aT»‡»?Aé‹ñœÒ?22aT»‡»AGN4FGL J1747.2+4937?Уløb
"@>tºËB‰À;wNÍÃlÒÀ<Ø[¶	;é@!
ì‹?ý²X''†?ËsyŸSAñ? »`=ØS?Տ¤ÐÚN@Ai'^è¿ïÿþÐñ?ïÿ±üfîL¿å5=߉'æ¿Ö3)"89,¿Ùð«C"¢¿Úœå¯ºAGNbllRX J1747.0+4938?ïÿ"Ôb{?cl~…cR?ÊÙ¡"Î?cl~…cR?ïô&'^?^ßddè'Á?W³Âýý"˜?^ßddè'Á?ïï˸XT3?krÈV;è?`4G†¯ž?krÈV;è?ïücöµ?%w&Çr¬?<àN4ÏEý?%w&Çr¬?ïÿšJL2?،r§?	mláäR;?،r§?ïÒ=÷¡&?|ð
Œ?vð`ï'ÅP?|ð
Œ?ïíÄ£ªáã?q@oØH?b;\˜vtÍ?q@oØH?ïó>ÇÍà?P1)l¯±?Y'p½Â?Ã?P1)l¯±AGN4FGL J1747.6-5308?ï·-s€«6À)/ñù¬ÿ¨À:oëBÙÏÀ;ö¶
¨@WS(q
^@~=½Ð°‡?Ä!_÷«¿ˆ†ê%´V?Ãì­è±î@µ›[慱¿í¸®6Ý?ï\£¥¦î¿ç{]U¹¿é6çRŠ¿ÖæÙ¾L×I¿î•¼Ê÷	·AGNbcuPMN J1747-5310?ïþ'az? {/Mú	?&îÞ*Ÿ‰i? {/Mú	?ïòí¢§¬¤?`náÿá?Z$º4ôÈL?`náÿá?ïÙ»ž.ÝA?qúž£óý?s"0ô@?qúž£óý?ïþg`P;›?×ßèeä?)‰ýP5¸B?×ßèeä?ïùJªÚDì?FéÅçºh¹?JÕU•uÆc?FéÅçºh¹?ïÕܟ—yH?'~{øI¥?u°'äÄ:?'~{øI¥?ïš2Vr4?Š[±ƒO",?‰sjm͇	?Š[±ƒO",?ïõÖUN!?KøDú›b?TSÝ-m¾?KøDú›bAGN4FGL J1747.9+4704¿£µýE™õ@=ù'ÙýÀ;VTÊ\°À<À¿\¢˜@¯d'`—ð@é?^º z?Òu{{vn?ã–]O@	uü wnÌ?ÿ¼–ž½p?ïçÝ>´ñ¿Õ±¥^ɹó¿áÊá:B.¿é™+€À…¿áà‡_rV¿çÈQY•AGNbllB3 1746+470?ï|ՉðëK?"âÝèÍx?eNÁ▖?"âÝèÍx?ëãAŠRË?ÀdåO[?ÀrùÖ´ñÔ?ÀdåO[?î"ìnRÃò?•!ß«&¢?¦Á9d$â?•!ß«&¢?í ã'9˜?š Ô‡'l:?¶ø罓ô¿?š Ô‡'l:?îo¬°š?«¡Gtg<?©."¡Ac?«¡Gtg<?Õ39ƒ§?Î4F/܈ú?åfz1c>-?Î4F/܈ú?é搁±µ3?²n"X"[?Èe½ù9+4?²n"X"[?Þw?Îæ¶?¾7Ãü¿¿?àÄ`sŒ¥?¾7Ãü¿¿MIXED4FGL J1748.0+3403¿íÌ_àÌo@@;-'d2‹À9ä3|‡À<h&£Ø·½@G¨Daª@Öé5¹q?»š¦c'?»'3`)¶]?ûÿ,ëñUB@ã¸cß"¿¦¦²Ü¶¤Â¿æƒ"Ó†û1¿à«Áïùø¿ãs[ýVØT¿ë¬»Ií‰Ü¿áË¡>(¯¢AGNfsrq3FGL J1748.0+3405MG2 J174803+3403?ïùKDeÏW?Fgq—'pL?JÒíô6Lù?Fgq—'pL?ïñLaÑñ?`µÏ´ûv6?]gæÓçþÁ?`µÏ´ûv6?ïw&»^C
?‡T'Š~	?'(ÈÆ?‡T'Š~	?ïò㘧gt?F@±^`‡ã?Z8Ï,ãÙ?F@±^`‡ã?ïæþð>§?h_¬=)9?iڞˆ ?h_¬=)9?ïÃØííY?…ÚÄÁ—bÓ?~"r[ç°?…ÚÄÁ—bÓ?ïŠÚÓºk?b_"oÈ?IK#‹ê?b_"oÈ?ï۝ԚT?`*ü-¼""?ru0óV¾?`*ü-¼""AGN4FGL J1748.1+2702¿¢‰=AY/ª@9‹¬q³À:Ð	sFHºÀ<~Êl <@"êƒÁëó@­[î=`?¿ûòTEÒr¿¥QÑìqX?çÛBEõ­—@F´\"~Ϳ蝘—;ˆ¿ãƒ¤?9ü¦¿è–Òª\_|¿â'¬¸ZO¿×™ŒÃó4k¿àÓ¸^€¾×AGNbcu3FGL J1748.0+270187GB 174618.6+270457?ïþ´
*°?bo¸¢$!?$¿Y É4?bo¸¢$!?ïê}³p@–?m^ñÈDÕÛ?e'L¾z¼?m^ñÈDÕÛ?ïð!I7?pT¬g˜
Õ?_ÿ¼ä!}(?pT¬g˜
Õ?ïý¾ª¨¾-?`‡µÜ']?2
©j´·'?`‡µÜ']?ïý<qã¦?2öî€K?6R¹3?2öî€K?ï´Õ…`°"?‰ùÒÒ:îë?'Êž©‹Å•?‰ùÒÒ:îë?ïä£:­%?{¨y³Â?k\ÅM[ŽU?{¨y³Â?ïðÖT5{?R¹=Gb?^SWSð‹M?R¹=GbAGN4FGL J1748.5-0854?×^ÞutSí@#O27Š°ÉÀ:…#\%šÄÀ;ݐZU¶ì@!Ÿ¦HÈF@—:*?ÃIƒ—#ȇ¿ŸŽr@†¥C?à‡ˆàcØm@^ô¶uÈY?ï"ùV˜"	¿æÐC¿dT¿ë4tF"ú¿Ó§;cƒ¾¿ãºua«ì'?Å/D%ɾ%AGNbcuNVSS J174838-085435?ïå?Xõ(z?•`Æ)Ø\?jÀ§·ý¤?•`Æ)Ø\?ï­6$\ß2?'â­0úÃ?"²vì7Ϗ?'â­0úÃ?ﺖãB_?®/ªèv?ZG \`8?®/ªèv?ïá1Ÿà0?U$•»²€î?nèÎ"FØ«?U$•»²€î?ï'*I!('?'áu3/m±?‹um­gÊ?'áu3/m±?í1q›4	®?¾ì|PĤÆ?¶ts(€?¾ì|PĤÆ?ï4nÍp¿8?—Vm¨'ž3?™r&P0Jõ?—Vm¨'ž3?ï5$¤q†M?‰f÷¹h«?™[kqÏ6p?‰f÷¹h«AGN4FGL J1748.6+7005?ïÿÏ(FÆ
@>¶–¢nTqÀ7×m̌5À;s;BÌ-k@ðˎkß?ÿ>(	3…i?–PÕZîu?¨Œã¨±d'@'
¹t*@-…Æ}þ¿•nZ·Â¶¿ÚëèÜLòw¿áaÚ«¿ÝóÂo{¸Þ¿ãO¡ÓÏË¿âäî—!ðAGNbll3FGL J1748.6+7005S4 1749+70?ïü3,Û³Î?<l¢Xc?>fšð-
x?<l¢Xc?ïôci±Êh?[ØCÀJ£?W9,·èÿ?[ØCÀJ£?ïç\x¯qÑ?lâ8HÀã?h£‡tç¢?lâ8HÀã?ïþWËF?·hÜÊ
?*£ÚÃk?·hÜÊ
?ïýΩéx?(Å='¢	®?1Š®Æa‹"?(Å='¢	®?ïÊuz.?€«!—?zÅ|;YÜ6?€«!—?ï濸ÎNh?yŒS÷€*	?i@G5÷á?yŒS÷€*	?ïýkÓ¸¤L?,c°s›"?4¡aV*Õ÷?,c°s›"AGN4FGL J1749.0-2327?×8§9t@­¯ÑƒÀ9"¸'ú
À:©"ðÅÐY@÷i¼‡/_@KUhè!?Û¬kBïó?à›q«>Ì@GŠLáZ@ñ҆õýô?îíN·ó÷´¿à*èÁŸòú¿ëÝõéüˆ|¿îç}R;6¿Ð6'Τ=b¿âGß½•LAGNbcuNVSS J174940-232619?ÔZ¼—©?Ô¦ÛÝ{?åðÒ¡´+|?Ô¦ÛÝ{?ÊÝa ©‡?Çc€Çªgâ?éH§·û•ž?Çc€Çªgâ?ã£^ ò"Ü?µþhzМ3?عC¾ØI?µþhzМ3?æ£~)'%?»(±yV¥?Ò¹­Å±·?»(±yV¥?Öì?ß n?ÒãoPè?ä‰àvoÉ?ÒãoPè?ƒ>–W5?',ÐÍË?þ?ï³½ŸÄg?',ÐÍË?þ?ßè›&?½"ÒÁi¨?à}qþ2m?½"ÒÁi¨?®îõ>ü',?±-0œ4f€?î«ôºý?±-0œ4f€MIXED4FGL J1749.0+4321?ëÜoxo
»@=&éÝ~˸À9:ªö¹/aÀ</ë/³L@j©t@lŠ½]Ä?¨–ºÒ܏?¡§¯†ëÂ?õ꾅m@"ý™É?O?ʞΌÀmC¿â4¤ý¥Ý ¿â‰ôafL¿à"IÁj"¿ã%"R¿à–[@î\¿AGNbll3FGL J1749.1+4322B3 1747+433?ïýý0dCC?ÿÊelÖ?0|HÖq?ÿÊelÖ?ïò4¡ƒ"?`:
IþNl?[–¼…"÷:?`:
IþNl?ïø*qvB…?T{1ÝDTž?OV9YæÖi?T{1ÝDTž?ïíÓCD´v?P8ì¼Îì?b,¼³yæ?P8ì¼Îì?ïüW1J?5â=D›ø?=Fu•ck?5â=D›ø?ïÏ:‰OÜ?€f͋Ûã8?xb»=°ž?€f͋Ûã8?ïøEÅö³•?ZÊ
g¸8?Nèèõ¹?ZÊ
g¸8?ïØmÎò?cõÎNÞ.§?sÉ$Tß[?cõÎNÞ.§AGN4FGL J1751.5+0938¿îyv¹oÎ@1¦»#WÀ7ÃãiÇC÷À;PáK	Î@ ‰ôµôï@'òeÊ?šã[üÍgõ?¹^Þ¡zRp@;'—•@F]	pl¿Ç'*t¿ÜmùÞýQ¿ãØÊfÀÿ9¿ãçހÔPпçL¢Ûa»¿èMÄC'OHAGNbll3FGL J1751.5+0939OT 081?ïí"§Â¿?"UÛUP?bÝXQ A?"UÛUP?ï{D¾T?£@f+ëܬ?—}meŸq?£@f+ëܬ?ïÉ7åR2Z?'ãƯÃy×?{d
T×Æ?'ãƯÃy×?ïù2¿4?=R<¹	^?K7Ÿ™?=R<¹	^?ïôŒì"oˆ?Tî9¬–?Væ&½gÅ?Tî9¬–?í±"g-`¶?¾kœcÖòž?²sÜÇíÍ?¾kœcÖòž?ïǶ
©Çö?…/xÝ¥	?|$ùMÐü?…/xÝ¥	?ïãþnÒ½õ?`¶†žoM?l')"ƒ!?`¶†žoMAGN4FGL J1751.6+2921¿ÚO=æÛí@9†¹ÃÀ9øzYbqåÀ<÷­K'F@Ÿ6²Á@™WÚ²h?¾ólɬÜÂ?À½oø
",?þ7Ó
ÔoX@3Žk¾"?åÞ¥µ%ç¿â"Px¿è=AÞËÓ¿çþ~pHg¿ë>¥Œìâí¿ïù‡ÀÔ AGNbcuMG2 J175143+2921?ïû³ë}?;¥†ã-â_?Cý1;犏?;¥†ã-â_?ïïmù­«t?f:u•Úýz?`'?»¸?f:u•Úýz?ïלÏ≀?sGµ‰Îî?t1—ö­ü?sGµ‰Îî?ïý X c´?#·œÙ÷E?6ý@ÛXµ?#·œÙ÷E?ïðy"ü(°?Z}…X¾a?_ö¬ò?Z}…X¾a?ïÁp¦cà?ˆNœ-8@?G¬»''?ˆNœ-8@?ïqo†ö?'ҁ´…	?'ÜHš?'ҁ´…	?ï÷£JGvâ?B!ÊLÁÜ?P¹k4™A?B!ÊLÁÜAGN4FGL J1751.6-1750¿æ®†f@?éúÚýÀ9¤±ÓLBÏÀ;t<"¸@ ,šä"@¦ÐNaŒã?¾&—Ÿ-¾? […â­‰¼?ål"¹™@׏SD ™¿ïƀW~A?ï÷a–5¿åZWBÖ>¿ä
º}¿ÉY¿â"ö¥
k#¿×Ïî,ëñAGNbcuNVSS J175120-175112?ïæY}Ûß?cX,æý?ib¦'$ à?cX,æý?ï–&P)l?¨»ôFë>?œM;<Ú
?¨»ôFë>?ïZXºÅþ?³y¶ò'Q?"¼"æïrE?³y¶ò'Q?ï}·'Ûœ?vIrs'¯R?I©ÆVt?vIrs'¯R?ï<qå|?™¶z9§Í?Ÿ¸qÅþ'?™¶z9§Í?èê·'aö?ÊwMDèx‹?ÌU#cîx)?ÊwMDèx‹?î‹šÂ'q?¢
ôšë?®FVq=ê?¢
ôšë?ìÃy‹v?§4ë;š?¹ãä3¤Oß?§4ë;šAGN4FGL J1752.1+4531¿ïë薁â@=Îg×®À;%3BEÀ<†#mÃQú@Çkcü@¨> N¿?ËÀ#8?²šð €Wm?ä^¯¨Ï˜@ø&¼x{?ïþ°_-âç¿Ì7ªçݑ¿ëênió9¿Üc—¿yÓ¿ïh¿ëxá=G3AGNbcuB3 1751+455A?ïõ©TD\?M£šeÒ±?T­Wö8ç_?M£šeÒ±?ïÜh"Ðk?xó*%ËE?q˵†Æ>y?xó*%ËE?ï…ÑM¿?"—Â}3I"?Ž‹¬›ÿÐZ?"—Â}3I"?ækü ?mè<x®øÞ?‰Ÿ†WBh"?mè<x®øÞ?ïԗ.Z[k?x‰1HºI?u´hÔ2"c?x‰1HºI?ïl‰uV¨?˜–w,0?'nÑZUTÿ?˜–w,0?ïJºÂoaô?'Gu9±à4?–¨§«4‰?'Gu9±à4?í$‰¡Öû?¡ê¹TL?¶Û²öÓT¨?¡ê¹TLAGN4FGL J1752.2-3002¿³—áðM¿üøÉZQ….À9]ʊÓ-9À:""д¸Ú@f­éê*@RaœÓ
?ҋ$÷0M¦?Ô½ÝüJô?ÿ€|¬ùÈ®@LH6z?¿_&¿ë¢AsgÖ©¿ç¾BuE|¿êY`úÛ4¿ïís 3*?ïH™"º]AGNbcuNVSS J175230-300107?î¥2k&?¹…¶¡Ÿõ?¥¬ÙQëZ,?¹…¶¡Ÿõ?ìüæ%?À6óe+Ã?¸ﷄýZ?À6óe+Ã?ç_•µÅ…l?µxô:`?Ñ@Ԕtõ(?µxô:`?íŸóôÀ?¡UuùŽ?³`Y'SÀ?¡UuùŽ?îµîìSÈ!?´ºBú*;?¤¡:Ã}÷?´ºBú*;?áÕp
»+?՜&­F}?ÜU×ꉪ?՜&­F}?â&Û°"0–?¶©ÛãV5?Û²Hž÷žÕ?¶©ÛãV5?Ñâã¸÷ƒ?Âò"3Ì?çú#"??Âò"3ÌMIXED4FGL J1752.6-1010¿ÎË÷¯úY@ K›ˆ‡"ŸÀ9Íj'E'À;rèn@P(Ð	˜@C@ˆÊ>?Îľ ¹?Ú &5j@Ž"mR?ÿ¨]—4åe¿æ½8:1
?îß®áÕG›¿áÙaÏ©¿é…V`߾¿äõ³;+¿ß«©f–7AGNbcuMRC 1749-101?ï°ÙÀêÛ?œ–J6?œIäÄs¢?œ–J6?㼶ÏÒ?ίoûÊ?؆"Ðà`[?ίoûÊ?ëøÿûÎB?¥;>™"›p?ÀÆ÷¡?¥;>™"›p?ê9ïGL	?¤':½§Q#?ÇCòâÏÝ?¤':½§Q#?æT}Ä®?È"KhwýV?ÓWwø£Ú?È"KhwýV?©À¸íFë?Êò™Uà)?ëUÑÄ®E?Êò™Uà)?ã£9l`•?µøÔÁd™?ع'>Ö?µøÔÁd™?Ïâ;ÿŠ;?³
ÍNü?èq\1?³
ÍNüMIXED4FGL J1753.3-3325?Úû|Ë`DÀ
ÐãF¶žÀ9¡Åè¬ý$À;–÷z€Ï@F³ÓÃt@uêgèG?ā¨÷…ˆ?âç@Áf<@w–¿Ê…Ë?ëX{-a¦Ó¿äBxùæá?ïøkç¿à	'Ë û"¿çM}™ù¿ïDÀ
¡©?ν{¶"¶ÞAGNbcu3FGL J1754.0-3321NVSS J175308-332637?°‡"¯¾…H?¿@Ô±r©@?íïª/W?¿@Ô±r©@?Â#›Ý/Š?ÁÀ'd|^ÿ?ëw:Ù´?ÁÀ'd|^ÿ?ÇÍ"'¥¿?¬½É×?ê 7v?¬½É×?°âòÉ÷?"°3'ä?íÿã¡¿FÁ?"°3'ä?™²Æç/¤ˆ?·¹;yÂ}'?ï2iÉ;?·¹;yÂ}'?—öƒ|E'?¡Ð;ÜÃó‡?ï@KäHÙ'?¡Ð;ÜÃó‡?¤—Ÿïû?™àwºÑÂ?óAß?™àwºÑÂ?Tz¦Š´?DF¥ü*Û?ïõÂöùàÆ?DF¥ü*ÛPSR4FGL J1753.6-5014¿ïH¯p4_GÀ(3¿ÂÀ9q¾íæøÈÀ;ÈLáZ"‹@™Ìs™@:œ£9V?·íÍ9Ú?лWYƒ)@ó ÔƖ@@Ÿ7=Xü?ïôT›bÇu¿áÔX<×ø¿æëªÞe{…¿é
áSíh¿î?S‹˜¿ïþ7=ƒï
AGNbcu3FGL J1753.5-5010PMN J1753-5015?ïY±´î^Ã?œ'òŠ·Ù•?"ÉÉ[Tï®?œ'òŠ·Ù•?ïߙ=SG¦?†ck‹ô}[?p3aoÉI?†ck‹ô}[?î:ÆÜ·•G?ž˜ÅV"j?¬S'3ªÄ"?ž˜ÅV"j?ïù"‡$³$?5øAwž?KuãäçD?5øAwž?ïY"¥/"°?ŽQuÔȎ?"ÏkS.R?ŽQuÔȎ?ïbo8œÿ€?ªU^µ¥»Q?"²ãÉ
?ªU^µ¥»Q?ë扭¤y®?ª<FšR®?ÀeÙInI?ª<FšR®?ïÝxpv'
?`8šôãV?qCÇÓ-W?`8šôãVAGN4FGL J1753.7+2847¿çþÀ묌@8tH@árÀ:écO͞À<SuDO»)@'°
ú> @Ü@Þ¡,?ÍÎ#äᖈ?ÁPý¢}C?ô'À®9@¾·ëêl¿ï¨"¾é_U?í4nfåè'¿æÍöÎ(Ÿ¿ÜI¹à<¿å'¶þ.o¿ïÿnªØ†>AGNfsrqB2 1751+28?ïýüo=O?.E
¹€…?0‡ñ®Ø5?.E
¹€…?ïçPÝú-?v¥QTy³"?hú¯ÆÃ#?v¥QTy³"?ï×qía?tƒ?Xd)?tGz"êëc?tƒ?Xd)?ïðb҈#?F%$C­‡?_Í:Ü!
?F%$C­‡?ïõÁ´Q&?Xq‰¤ÀÔp?T|—å4µ?Xq‰¤ÀÔp?ïòÔ@Æ?˜ùsåN$°?Œ~D–Ÿ?˜ùsåN$°?ï?ßâ[ÝÕ?•ÂëûÐÁ/?˜­¥
m?•ÂëûÐÁ/?ï™SÀ
`p?~gP¼É?‰«¶·õ?~gP¼ÉAGN4FGL J1754.2+3212?Ø"Ÿíƒ@9hÇ\Jƒ²À8|'¿bÀ;'=mHØ·@üµ‡‹Ð?û÷BÖ>f?¤v3ãÝ4¤?ºüYxûê@'V†''@°Ž'ºR?èÄHÏ|ªv¿ÜØP÷¬¿ÖL˜_¿ÜšäN¿ääúœ>¿à#Ü~¸AGNbll3FGL J1754.1+3212RX J1754.1+3212?ïúáhmÛ-?@#•0'Ú?Dz]ûMò?@#•0'Ú?ïåoýÐ?vòÕÏo´W?jþæ³ú?vòÕÏo´W?ï®}6À+?‡dpˆ$è?"`²Q´C7?‡dpˆ$è?ïú…6'•h?4æ½}Ù ç?Eë$ý-Ä?4æ½}Ù ç?ïûöº±í?>Œ3‰ûP@?Aø%GÌ$É?>Œ3‰ûP@?ïh;iÒEv?¯³Ù¦mö$?'ø'½ K>?¯³Ù¦mö$?ïÎý"‹"û?'ÎÕJ%¼H?x6QšÚ;?'ÎÕJ%¼H?ïô•}%?FÁ®n™?VÕ»vo?FÁ®n™AGN4FGL J1754.5-6425¿çwck+ÙÀ2yhÍJ¡À:÷È#àÀ<:©€—j@bÕ~w)W@B:73s?ºŽ4`¯Ã'?ºOM:ö?þ,—£TY@›ºø9;¿Õ6³t¿àTΎmìm¿æ²2í"ò¿æ/
¯†k¿ç¾;]e¿ä1RB˜AGNbll3FGL J1754.3-6424PMN J1754-6423?ïü·ÖÆuÆ?0($\±ú	?:AJ–¿?0($\±ú	?ïî"!¬ð[?k,çP›ø¾?akÞr¬ë?k,çP›ø¾?ïêÜÄ+?oy›*.?e<cãž-O?oy›*.?ïèbö"P?N"¿4@ ?g	ØrO¯?N"¿4@ ?ïóUû½¯?S]cÎՒN?YÙT5Qð?S]cÎՒN?ï½4e&9>?—]©E·ƒà?€²æ¸)~^?—]©E·ƒà?ï²tÁjeq?‡#¯m{?ƒbϖ QÚ?‡#¯m{?ïOjL¿?"¨eòõ—?–±X^-?"¨eòõ—AGN4FGL J1754.7+3444¿æÅx'®‹@:
~À¨À:ÉÕTZËÀ<YT¹•¸@Q]f¸pÊ@Ð_ÿD^?Éþ¬˜ÏÅ%?Öèè÷¥¾k@×èÚI@¨þoÝ­?È+Ê^2K¿Îy™ßd©ù¿æ¬¾´ .¿ëOÀ²0¿ð?ìçìãÉWAGNbcuMG2 J175448+3442?ï쾞@.?uýŽ ì?cAøR¡Šl?uýŽ ì?ïìÏõSÝ*?h—ƒ£èÄÑ?c0
Ú݅O?h—ƒ£èÄÑ?îâWM…€?"NǕ(¼O?¡ÚŽœßuü?"NǕ(¼O?ïù(4ýbÂ?8-BªB{?K_,çuqb?8-BªB{?ïùÚnöغ?Wщ°z ?H–CIϓ?Wщ°z ?勞I¯ "?™.xØ;½\?†Ô-"7Úã?™.xØ;½\?îX–¥Qq?èc :"?ªv•¬¦Æç?èc :"?ïÌ+<CÓ?n!Xƒdz?yêaù"V?n!XƒdzAGN4FGL J1756.3+5522¿Íׂ©Ž@=¶ê šª;À:€~?¡À<e–È.›@ a®.ß<?ü6À5¯å?¶oçnŽ¨û?±3nÂUz†?ûgÿÚ$@æ~ÜÿÊÑ¿ÉîRCÙk¿ä s"6‹­¿ã€í0£?¿Á5µÙì¿ßÖ÷¿àÏ>šõ9AGNbll3FGL J1756.3+5523RX J1756.1+5522?ïþõôŽ\Ð?«¤WU¨?  º+@)8?«¤WU¨?ïò'ý¬?b4'†Y?ZûÎ[,øb?b4'†Y?ïú'2Еb?2¡¸ž"4?E·3ÜDÑ?2¡¸ž"4?ïñ°°Ñ2|??þlm}IÒ?\žžœÓ×Î??þlm}IÒ?ïþX"h?"¿Äòæ‰?*vÊÍ€Z?"¿Äòæ‰?ïÔ "A?Þ?yb²¥H%?u¯îƒYO?yb²¥H%?ïúëdx¶±?RÒÞúÃË\?DRnKßêÈ?RÒÞúÃË\?ïÕïgνµ?a±§mÇ͗?uL#…?a±§mÇ͗AGN4FGL J1756.6+1553¿ê;"´Ñ.@3PÅë1<À;ۉ(2NÀ<†@Š3Ë	@!M•¨H^@&IlÊ.?ßËƽi,"?î'­ù¢î­@ñ'À8iÔ@i@e˶Í?ïþ@Bo	¿ïü­?"¾¹?ï‹4|¿·^koe¿ääc1Ù¿æ<ÞÏ®©AGNfsrqPKS 1754+159?ïÔQbÀ‹î?€—4±ÚÐh?u×N€¡?€—4±ÚÐh?ì¸<
?Ã^t	g1è?¹ê?¾Ϙ?Ã^t	g1è?îûqeröm?"E|ác? Hé«dN2?"E|ác?çÁ¹pÇ?¸˜îä¼½?Ðä}čr?¸˜îä¼½?ïÑîhí™?€æÍÚÿË?wËs5ø¥?€æÍÚÿË?éßTõáÕ?Í¢çԘ§?ÉȂ¬(x«?Í¢çԘ§?î3:®Ác? 81[Øóì?¦üÌPÈfÙ? 81[Øóì?ÞÊCÒà?È´ÞÖ?àõޏþ?È´ÞÖMIXED4FGL J1756.9+1531¿îÇú˜7ñ@2æãæÄŗÀ:ðHG—nFÀ<b.bT@»ÃZ]C¨?þ³(fP–ñ?Ôào Ê$ý?Ñ¥7<WI=?ÿZÐeށ*@lÏ,M'?ïn+÷Տ?íû.t‡'Y¿ìp2˜Á?º °º›í¿ïÿÖ_Æ	?ïú2–UA{AGNbcu3FGL J1757.1+153387GB 175437.6+153548?ï×>ž‡?tF:ƒªá?t`ø}°b?tF:ƒªá?ïNP$T?§+5ïÃJW?–5ý¢^u?§+5ïÃJW?ï
Øjå§?'(vš7»?žDò«â$+?'(vš7»?ïšîT?ž?v¡ÓV$ƒ?‰Djú0ˆ?v¡ÓV$ƒ?ï+"È×Ê­?¡¬ôþ	Õ?š›¦Þ'rs?¡¬ôþ	Õ?ì
Ý²š"?ú1$÷A|?¿"ñk+a?ú1$÷A|?îID'?ž
£ûžý?«k·Þ#y?ž
£ûžý?í¸uNîG?¨T†ÆÈ?²<WKпÊ?¨T†ÆÈAGN4FGL J1757.0+7032?ì·L¥þŠh@=ù…H©¼ýÀ;‹y¢ƒÀ<©ô§Ý);@!· ê±9H?ûI>‡û¤?ɳû*-P?¸4tѹ?ðK'ëk:@‰LC$—å¿ïêKÎ4«Ù¿ï']Àz"?︶•Râü¿Ø˜±ý""¿Ý/<Ùz/¿ÖAW›:ÙAGNbll3FGL J1756.9+7032MS 1757.7+7034?ïÿ')ì@8?1¡ît%¾?u"sj1F?1¡ît%¾?ïö¯TŸr)?Séã²?R¡V m¢?Séã²?ïù›`"¥?=k6ÖÇÒc?I"öQ)°L?=k6ÖÇÒc?ïö~9@éT?AÌbæåÐ4?Sƒ¬·t?AÌbæåÐ4?ïÿ§2¼ôE?›PÈ
20?3Jî<B€?›PÈ
20?ïÓ#ü½?{Ðׁ-R?vn\o^?{Ðׁ-R?ïõ:°?qâÄïªf?Uïõ¦Ð>?qâÄïªf?ïíFñÅÄ_?Xî¹×]¼¢?b¹v´Àþ?Xî¹×]¼¢AGN4FGL J1758.2+6532?âi ç…y–@=ý)WÉÀ;K³ò
s÷À<¿ÇòrxÃ@ûX4õU,@åùÄ|œ?ՑBq>²?Ú*–ÁøÞN?ëáÉ^-\Ú@¬Ô=Y|É¿ìA#`Ø2¿Ó‹ûKeY ¿ä×	 åþ¢¿æjK˜"Ƥ¿éK§ž?¿Ïž¹(«õAGNbcu3FGL J1757.4+65367C 1757+6536?ïØÊ
òï™?­Aœì*"M?sšúv¹ÿÅ?­Aœì*"M?ïòæ ø!~?YH$Ž'Ñ?Z2¾NõÓw?YH$Ž'Ñ?ïDÁÕ;Êö?‹G·Lþx?—gÅ[ö=7?‹G·Lþx?ïàÓÆLfF?TöÃ0åÓ?o,9pAb?TöÃ0åÓ?ïÝdC:V,?n3RÊno?qMÞvÂ¥ê?n3RÊno?ïÅކˆšÄ?z˚ໟ?}¼²Ã¢/?z˚ໟ?í}£Ú:H¦?¢_B+®?´á,ãàP?¢_B+®?ï3 ïñÀ?…ªÂ+¡(
?™›ý›"?…ªÂ+¡(
AGN4FGL J1758.3+1429¿êôãaJå@2.ä¬yÀ:'¶ªK˜…À<>­j0öB@®­€VQ›@ÍæÝð
¿?ʞÌßAC—?ÊÑJµÛČ@t¡'Œ_@dlH¨W?ïOÇão?ïþ"û¥'l¿âݸ½vB§¿ákßj‰6¿âøÀ$óª¿ïü;±îAGNbcu87GB 175603.3+143022?ï2´Gżb?±,5§?™©w
¸²?±,5§?îTr'«?²Æåo?…?ª¸Öꕲ?²Æåo?…?ï5ׅ&?"îø–‹9ˆ?Œ²¿ÔmŠZ?"îø–‹9ˆ?î¦Æ§³|‰?ˆqáˊÎ?¥"•ƒìPy?ˆqáˊÎ?ì«dx¶±>?µfá
ã?º¤Ü:Jv?µfá
ã?è¶{ã·[?Ͻ4™I?Ïå&q""?Ͻ4™I?ìGAÓ½Šm?¯[ÅÓ¨@ù?½Åñb¬–?¯[ÅÓ¨@ù?é;rÛ¾œ?²ú[Z¬d?Ë7´'?²ú[Z¬dAGN4FGL J1758.3-3028?ïÛΘE À	VDÿäQÀ9‡¨ÖMÀ;$Y'¹'m@я‡G¥@,&Mq£?»J}ãÁÂ?»&@Üi"@¦¿òÉ·@λÁÎj¿Ú—"š|©?ïòZ€T#C¿âž/`?Û¸¿ä¿ó5bB¿ç(§ß, È¿áå˜îxïAGNbcuAT20G J175822-302916?ïô¨åÐ÷?c^Ü·Ùÿ?V®ÄMA?c^Ü·Ùÿ?î÷fö¦‡`?¤èhh,
á? ‰''î?¤èhh,
á?ïƒ0\ÐL?"qôz¯?o™ò®(Š?"qôz¯?î˜ÎÃûuŠ?‹€!ñ«?¦sÂuY?‹€!ñ«?ïKì°s?žˆ`ζ¨?–žâcù¹?žˆ`ζ¨?è@úû¢z?Íþ‡"&N&?Îü™v?Íþ‡"&N&?í]Øv+Þß?©³žiÂN_?µ<Oêã‰?©³žiÂN_?è^l	=–d?µ——>*?ΆOÛ	¦r?µ——>*AGN4FGL J1758.7-1621?ïm²Žªu@aXPÀ9œŒ…´àGÀ;qõ *­S@±€k^@*ˆŸvRm?Å ùIØf3?ÝÁæßóp%@ªò×ùP¹@	Ré¿KÚÊ?ïÓíözE?Éà+yUg¿æ™U ÃÄæ¿è	ÿþR€Ö¿ïÿÿ^ðP`?îÈË ÒÈåAGNbcuAT20G J175841-161703?ìW?þYQ?¿Zutÿ¹è?½Fx
5{?¿Zutÿ¹è?ÝKsé(E?Ñm3¸Fán?áwZFkÞ?Ñm3¸Fán?æ7`ýóK?±Jüœîïª?ӑ>Êi?±Jüœîïª?ê9>F"?¬—†ÀŠ/€?Ç«åð?¬—†ÀŠ/€?⿚ö©"?Ï¡hV;Ý?ڀÊέ¼?Ï¡hV;Ý?›g&V‹9ö?­¯)ù£šy?ï$Æͬq?­¯)ù£šy?Ùú+ëb=?·¡ShCš?ãê
uNâ?·¡ShCš?ÈN™¸o¿ù?²¾iÓ³dÕ?éìY'ä?²¾iÓ³dÕMIXED4FGL J1759.1-4822?Ô±/QkÀ'èE™gD³À9€ƒmÞ*À;úŸ[zz@Õxèt3@µJd¨ E?¸5hÀÞ­?Â5záº÷@©]'«Ž@;;-Ržˆ?ïý› Ø<¿×ÈIe#Æ.¿áñ"ý…ý0¿ä€|â©­ä¿çåöÔÞF¿ïÿö?ŒÝÉAGNbcu3FGL J1759.1-4822PMN J1758-4820?ïüWÀõíÇ?8ERæ˜ì?=Aú!©°¶?8ERæ˜ì?ïîxÏR@È?n¿²$Xd?a‡0ž ïð?n¿²$Xd?ïǎsîÏ?}¥S¯}"?|8Æ}¸?}¥S¯}"?ïþÂ0ø¬‹?*ÓMÚ?#ÜðI<Sª?*ÓMÚ?ï÷`~ ±?PClPB?Q?ÚíÁö?PClPB?ï§jë0e#? éU‡…•¸?†%E&(Gm? éU‡…•¸?ï,ÄÜ`?"÷""æäc?šg|ÄSü?"÷""æäc?ïýåƒ§ë?&{å¤Jø?3Ó¤7á?&{å¤JøAGN4FGL J1759.1-3849?áñg>†+À«Då^³À9¼~Êá:BÀ;Ñ E…EO@³WÞcM,@pöºÜà@?À×&B	?Öæa~?¶@†®â:¸@Æïp:Ћ¿Å«.1Z¿ÜR€ vÿà©
?ƒ£Ž¿à4æÇIÖ
¿ïø]߯' ¿ì#;~†BÐAGNbcu3FGL J1759.2-3848NVSS J175926-384753?ê	€'5V­?Á›>{?ÇÙÿc*¥N?Á›>{?îpÂÀ"j?«½÷Œ?¨óÓö'Š?«½÷Œ?á—W" í\?´L'ªO?ÜÑPؾ%H?´L'ªO?îû_L@ËL?'Z g³? J@>Î6?'Z g³?ـ=¥Ûyì?ÌDqO‰¼=?ã?á-C
?ÌDqO‰¼=?æZQ'Ãq?ÎŅ}$e?ÓK]°yè?ÎŅ}$e?Ïv‰÷"º?·úük¦
N?è"]œ'?·úük¦
N?è%0ëҘá?°a…)Ä?Ïk<Pµœ|?°a…)ÄMIXED4FGL J1800.1+2812¿ê''"-ý@6îð8⟝À:ôSËY/FÀ<›'pˆ(X@ î»J™VS?þðk®Œp?ȸLHß?"ˆfývI?Ñmâ=ž@ÎëØ֛X?ë,yÀ¶>¿ç›¸䆨¿çî°ýŽ`«¿ÚUã ÷€¿…QU)Ÿƒ
¿êG¶þ.n¨AGNbcuNVSS J180002+281050?ïý⹞ß?*)O†}ŽÀ?0ê1'™4?*)O†}ŽÀ?ïíL/ó&˜?i"S}Ú7 ?b³Ð/5€H?i"S}Ú7 ?ïðÎØk~?mÕ7éG-?^bO…ð3 ?mÕ7éG-?ïüfï^ƒT?&Õë~x?<ȅs@·?&Õë~x?ïü+²`dð?:¿-·rd›?>¢mqdÜ1?:¿-·rd›?ï±m®.Q!?‡ž%ct–?ƒ¤"qT¸?‡ž%ct–?ïîæE!{?qa‹íŽ?apƒäÅu?qa‹íŽ?ïñ¯OíG?QÓv~CH?\¡b*_?QÓv~CHAGN4FGL J1800.1+7037?ëuBµÀI@=·hß½jYÀ:Ê,"ÜÁ7À<‰ep!@ ̀Pó8?ÿCxà¼mÚ?Ë+ëb<á?Ã;9&b?õàoP–@ôe¡o{ä?àœ)@ìt¿ã4>Kë¿â¼RÌU®ˆ¿ÝÜ›Ýk«¿êøU|3WE?´.FåA¸²AGNbllRX J1759.8+7037?ï‰ôà^œe?¾'䆸ýs?'Çï8º?¾'䆸ýs?ïô™ó† ?Y^GP§}?VüÌõ@E?Y^GP§}?ïÍHãý«?~ޓôì?y[Ž¾¾X?~ޓôì?ïå{}àç?J²,‹&ˆh?j"êÞS0?J²,‹&ˆh?ïù‹"C²î?J±@$â…?IÓv›ýöà?J±@$â…?ïÊæ¨7Ž"?€è-bN'Ð?zŒ«ÛIÂ?€è-bN'Ð?ï¹D«ðM?‡bý"M¬?®Õƒ¾]?‡bý"M¬?ï–Pér?q•"+å?Šzk´Œ—±?q•"+åAGN4FGL J1800.6+7828¿ï䌳›è@=‡¤¤—À7£>d¿9À;‹Àò£öë@ò@/E@Dȍ$@?'ÃX&T?¢eÀN9H÷@(T<j@™ü)ܝO¿ÎŠ'ûG‰¿áñ<ÞC¿ãΉ/¿
l¿á؞AŸÁ¿åd]½ukè¿év"U:oAGNbll3FGL J1800.5+7827S5 1803+784?ïýÜkȝ`?#­($Tô?1ŸàҖ?#­($Tô?ïõtkŒÀî?XVÌâ²?U)ùÒ?XVÌâ²?ïè%Îú,4?pi¾6¾L?gÚ0ü4ãô?pi¾6¾L?ïûHIÛ?6AÀ0€?Bßçb£ƒë?6AÀ0€?ïþš‰R"?§T$2?&^v¤íJÊ?§T$2?ïÒÒ]¸ö_?y¬ÉÒ:'¯?v–Ñø,Ä?y¬ÉÒ:'¯?ïîQ>ÌÄ?r!hŽÁo¾?a®p¾s‹š?r!hŽÁo¾?ïöÜrÝH?JW'Ð:úý?RGϞá?JW'Ð:úýAGN4FGL J1801.5+4404¿ÐQ¹1J¶ï@;Þüz9'À8±5
þÆDÀ;ò×DÁ@~$žÅÓ^@uçÈѕ‰?¢m!à?±ž©Š@µ›"/Õ±@§¬áB¿Ñ<&âAþþ¿áÀî<‰K¿æ¡¸í÷­¿ã¡ a}ï¿ê+h{¿åQU]*AGNfsrq3FGL J1801.5+4403S4 1800+44?ïüJ‡sãc?1¼­¨>×è?=«Ä‡`‰f?1¼­¨>×è?ïóN×(›U?]§9¢[‡­?YbQ҅Fo?]§9¢[‡­?ïæK?^ån¨UÿN?iùù'©?^ån¨UÿN?ïÿÛa²nõ>ç|כïU¦>òO-kí=€>ç|כïU¦?ïú¶•†m ?@vÇIÌ'¡?E%©ÊΡ·?@vÇIÌ'¡?ïƁ"n-Ê?'ºÖ¤=Á¿?|¿néåZç?'ºÖ¤=Á¿?ïÇ#߇'?=ÿB'†D?|nU?þð?=ÿB'†D?ïÿÖQµª>î"®wÃÌ>ôó_ß`ã>î"®wÃÌAGN4FGL J1801.5+2123¿ïp°ÅÏF@41GàiaÃÀ;½ôµÀ<Q )k3U@7œ9Üñ@ƤD‡?ĵ¤as¸¿§YÝÝÒj?å\=îx?ý3="šÙá¿¿—b¡y¦¤¿çí÷­K'¿å—ß_¡{:¿áÛ`C6¶¿ëOqºû?Ä}XEff'AGNbcu87GB 175915.8+212212?ïæ«?ß>?eF¢(ñÕ2?iT¿þeÔ¤?eF¢(ñÕ2?ïÊ	ÂT,?€Õž—*4¤?zûû>rR?€Õž—*4¤?ï¤ã…‡$2?ƒî%о?†Çç…?ƒî%о?ïÒ¡{ÌeZ?^Må
zÚÄ?v¯Aù€ÿ)?^Må
zÚÄ?ï¡NW.˜¢?€íøÃZé?‡¬j>¨«\?€íøÃZé?î[÷élPò?±'ÊHp?ª@gƒ"Þ?±'ÊHp?ïžP¤¡ú*?‰bV v?ˆkÖÞ`­q?‰bV v?î.Åv}q?™Í5s‡ˆ?­¨"¹T?™Í5s‡ˆAGN4FGL J1802.6-3940?ê•R#۞ÄÀ ×d­ÿ',À7†Ã!À;/kn
#Õ@÷ZšUVI@ºÞ¿q?›0œ]¡ÏQ?Àƒä%®æ2@!+ˆ‡"ž@ –žèc¿´õ¶6ˆR¿Þž K¿åH'NI9¿å±Wü@X¿éLõ‰¾¿ì¼Ý5МeAGNfsrq3FGL J1802.6-3940PMN J1802-3940?ïñQ³?̸?[g-!ó?]\™æþ•?[g-!ó?ï×Çã6¤5?"³pª?tFqUç?"³pª?ï"ÃËéšZ?Šåçó;Bï?‹
è=\?Šåçó;Bï?ïÿ
¯É^?…V©u}Ý?J
ÆF?…V©u}Ý?ï¢xqŃò?"ÓwX/?‡a㎟€?"ÓwX/?îkÝ_R\*?¸õ‰eŒ$P?©B*'e?¸õ‰eŒ$P?îÝY¸`·®?œ¯'@
?¢*dyô…?œ¯'@
?ïû379ýþ?=þQPhñÜ?C3#/?=þQPhñÜAGN4FGL J1803.4-6510¿Þ %šoŽÀ3¤çÝÊKÀ:Hð3Ú"À<')H>@åWáY@;hê?ÀyYÑÇÞ?ÁÝÀåãÊ@Y%5C¯@»ž;¿É¯?Ð$¿½o·ž¿àt•žbV6¿æ~|§ñK1¿é\VbbJοâonLå¿ïÿú@ùDzAGNfsrqPKS 1758-651?ïþqæî?""÷½Å\n?.xå0÷\ü?""÷½Å\n?ïóígՅ?Yãú峩]?Yð%Š»?Yãú峩]?ïäÅ*RJ6?e몌ö½ö?k:Փ˜Â:?e몌ö½ö?ïø¤)ç|?2Ó¡
¿?MoÞÀÅn?2Ó¡
¿?ïùê:m?F":­È?K°V÷ӆ@?F":­È?ïҖUÊëT?

úví?v´ÕmN:?

úví?ïˆ8­½àB?‰$/#ÿY?ñԍSt?‰$/#ÿY?ïÎü4nq£?g‡Ow/	?xå°	þË?g‡Ow/	AGN4FGL J1806.2+6143¿ï–OÀ»$@<ô¡7óŒTÀ:­FBÐ_À<ˆ¢üïªG@Y€Œ­M@ÒÆü©3k?Èg¨Z҉z?ÉqBãTy?õÏíé}¼@ßÿ/ögÑ?âXO'RÑ¿å9ž»'¿êi8"†<Æ¿êpBóš–ð¿î¼üJÈü¿ïÿø¨ó©°AGNbcuTXS 1805+616?ïûÃ."g?=zŒÆ!X?@ó¦lÇÀ?=zŒÆ!X?ïð{H~Q?mµ5ÊCÝß?_	n*6<?mµ5ÊCÝß?ïØÿd
?sõëÜáÝ ?sò|*²Ú?sõëÜáÝ ?ïÓ¹_ª?]¿M†9K@?v#PPÊí?]¿M†9K@?ïöµk(ºV?T)h¹¼Ì'?R•)χ"@?T)h¹¼Ì'?ï¼ßÚÏ!™?€â†ï‡/´?€È	G/¯?€â†ï‡/´?ï²xõ×{?ƒ<Fh€X;?ƒa™îU??ƒ<Fh€X;?î×$ÒG`?‹¹ñ'õèO?¢²ÙÒ0ô?‹¹ñ'õèOAGN4FGL J1806.3+5345?ï~a½4So@<²[1~þÀ:‡Ç™kvÀ<oaÊsc@³IÁ?%@¸;Ÿé?À×Î.äð?²Î¤¾:ã¬?íü¿øÓç@y³Ž¸?!¿æÿ'æFñV¿Øò­œ…Ý$¿æf~ºC¿éQæýz"œ¿ãI‰›á¿åݖ^%ÐAGNbcu3FGL J1806.8+5346TXS 1805+537?ïþõ퓧ù?¨ÑèÑқ? ¡$L.Õå?¨ÑèÑқ?ïôuhî?cNJøŒJ?W/d	%?cNJøŒJ?ïîkڈf?TGFfœç4?a"%tÚK©?TGFfœç4?ïûVjšÓ€?)s1gÿЗ?B¦VVÀ?)s1gÿЗ?ïþ$ÇúCí?)0ü·Í?-³ƒNš?)0ü·Í?ïÎy]#?yðm¤gå­?xÃQnŸª\?yðm¤gå­?ïåXáåÛ?rDÀK¤Œ?j§GϦ?rDÀK¤Œ?ïæYç/­?Xdi:"?i¦ܱx‰?Xdi:"AGN4FGL J1806.8+6949?탑qä!@=*½¨!óÀ8
|à%oÀ; ë)¯%ó@®MÈ_Ö@ñuù`¾?—òu"§¬?ª%û÷:@®›aöK@ÄÃb벖?ïý6Â3엿àùÛ=¨×û¿äõÔ-^'¿ãe.Í/ô¿æ].yÖ¿êo¸õs~AGNbll3FGL J1806.7+69493C 371?ïû˜úã5š?YåS|Œí?AœV6-€?YåS|Œí?ï謹©8?a‡åDu,?`U@gcèc?a‡åDu,?ïÔ>MÂK?|È¢þh?uàÙ"^bV?|È¢þh?ïŔŠCÃØ?iò׏Ը?}5ºþjg÷?iò׏Ը?ïý™y@ç/?3ð"±{®?346Øž?3ð"±{®?ïºF‰"Ê?ä4ËÎDþ?n]ÅÝq?ä4ËÎDþ?ïșXDÿR?ƒkïàHºº?{³S잞Æ?ƒkïàHºº?ï:AÓÆ!s?ˆlQ*ø£¬?˜·ÅÒ׏?ˆlQ*ø£¬AGN4FGL J1806.9-8038?݀IQëÀ8öt)ˆ<À;Vm¾iÀ<±>K•)È@ á'&³ý?üþ¾œˆac?Ñcz"ÛÍ?ÆqLN÷?õ,JŸ`ƒ@ƒ»ùë¾Õ¿éÓÂõ³uä¿ïÿ½ 	c?ïü•¢i!¿Ï虚eG¿ìTտ到?ÐÑ"D¿AGNbcuPKS 1757-807?ïø$žÐ?I#Gëz#?OomDé[?I#Gëz#?ïòÁj»W&?\—êAý¦^?Z}*O˜D^?\—êAý¦^?ï˜T3¢³?%ÏiΓ?‰êó
H°?%ÏiΓ?ïéd$­?YYâc~'?f›Û v9è?YYâc~'?ïö•@žÝ?Q¶ÒPû‰8?Rխƍ?Q¶ÒPû‰8?ïÓ¢áZ½?|^¾Î¾ž?v~®òÉm?|^¾Î¾ž?ïŠÍڝs?‰АMV?L‰nÉÏQ?‰АMV?ï³ìѤøÈ?€_WÒ\S?ƒ˧?íÔ?€_WÒ\SAGN4FGL J1807.2+6429?ïMb ±{c@=Gb• ŽÀ:øã`'À<רª˜@ !
]¦ú*@¿»lR9?¿
…&}˜¿ŽöjÍJÃj?юÖ<b0ø@	¼‡°8?¨šák.¿ÛJÿ"	•*¿â»uÝök¿Ó[<'¦¿å0¯?ž%š¿ã}|BםAGNbll3FGL J1807.8+64277C 1807+6428?ïÿ'U¤ð?*ÂgÀe?m­RÂ?*ÂgÀe?ïöñìŽ?VyâžW?SýÙ³²Ãæ?VyâžW?ïùþZ}=Ý?6QïúŒî!?H—œÝ>?6QïúŒî!?ïý꿯‹|?DŽ‹?u?0ª`¤˜}?DŽ‹?u?ïþ¡õCõ‰? sû˜ ¬R?%à«x ? sû˜ ¬R?ïփ`Xk?|S¬çµt?t¾O͚íu?|S¬çµt?ïüuDXR/?R.í
•?<UÞ×e'?R.í
•?ïû´0É¡t?.è͆kĶ?A/=Ô·7ƒ?.è͆kĶAGN4FGL J1807.9-6412¿ïðÐm"À3ºnCªy¼À:Mð÷3©À<Ò¡"$@b,™!O@Lë]±‹ÿ?¿bVz]?³,Û§?òö`ÿõE@ÿ@±K ?ïÍ>¬ãù9¿âĬ½bÌ~¿éñ9ÉOiË¿ãRžÓ•=ê¿èó2ýƒMþ¿ïÿôÕ÷AGNfsrqPMN J1807-6413?ïû¸z°J`?BI…°Õ×Ð?Aá?BI…°Õ×Ð?ïóåAží?YÚÓ«¥>?Xä5ö¥?YÚÓ«¥>?ïã'n.Ü·?e*Oej&]?l}'éàx?e*Oej&]?ïú·&zñ–?,N5%Og–?E#g!›ý?,N5%Og–?ï÷ACRvV?M‡CDµI@?Q}y¸ˆ´"?M‡CDµI@?ïÕW¾1\?€¯Õ0K´Î?uT7ž'¡ó?€¯Õ0K´Î?ï´ª)âÓ?'ŤïI?'ÕuºW¯]?'ŤïI?ïäçk''é?W¿&ÄÅù?k"4.õ?W¿&ÄÅùAGN4FGL J1807.9+4650?Ù·Ž_‡W«@:'ú'è},À;*ƒì‰*·À<Êˀœs@ 궦oÀØ?þW§6:N°?ÃÁˆ5™¿^…'Wîå?–V»ÅàÁÄ@K\YQ?ïrÿ0Í'f¿æþíþ¿Úw
"˜±<¿ÞÒÕºÝ3¿ÞJžß©žJ¿¶ìKÿC'ÙAGNbll3FGL J1808.0+4652RGB J1808+468?ïý±~e¥?$¹Í6<5?2wDDæ#?$¹Í6<5?ïô—óbsú?ZÈøð'Ù?VОÌ?ZÈøð'Ù?ïö±+L4?TåQ	$Dm?RœåT1H`?TåQ	$Dm?ïö¶8X.?5ß¼¹ˆˆW?Rà"@¤3?5ß¼¹ˆˆW?ïû·dEê?:&Ó	vÛå?A!Êùþï…?:&Ó	vÛå?ïÇ퀇µþ?Îrì?|	?¯}K?Îrì?ïø?–^?a-©˜TŸ
?OºqdI?a-©˜TŸ
?ïä=w]Õ?W_,àî?kˆUÅsƒ?W_,àîAGN4FGL J1808.1-5013¿äFp6ô³ÇÀ,.ŠqÞi­À:Öé†@÷À;ûŠŸb0@fÀ'¢Ü@‰ÉºÉ•
?¾r]?¡+?¢I=`³žþ?á±+6½+@MΛE–¿èÙÞÃð/¿Ù…=jĚ¿é§1½gT"¿çÉóïT6¿ÙÙÁY|¿ïþµ}$îÍAGNfsrq3FGL J1807.8-5011PMN J1808-5011?ïþ$æ"I#?'{b°ÛÓ£?-±–ãî'?'{b°ÛÓ£?ïóœx'Xñ?_'«K‰Ê{?XÇ®Vݍ?_'«K‰Ê{?ïÜ/<è¦?nCòß`AA?qèaÝþhõ?nCòß`AA?ïÿ,«"¨œ?&"Ûý"?j"–¼g7?&"Ûý"?ïüR%^*Ð?>êP'Å	?=nÕuL›?>êP'Å	?ïÖÔ0ï?{
ìÃdOª?t•òjH!È?{
ìÃdOª?梅aŠDÎ?…*NŸl$?…žç–"?…*NŸl$?ïû@Fìù?;a>U¼?Cúþ̧N?;a>U¼AGN4FGL J1808.2+3500?×Ëãî§h@7uø>ŸÀ:&ÀMb‰bÀ<=JYPÔ@,'úÅÙi@ÿ:Þ"_¦?»7ðÝ"Zs?°_y[X?ó;ëh™@	âæk"?ÄZ÷ÝǛà¿äIÜݼY¿ä&»‹[é5¿áHí¯›d¿ëª¥Gá@?—Ÿ÷y7AGNbllMG2 J180813+3501?ïú'D4Ú ?=Ž°ïÓ?EöðG
)?=Ž°ïÓ?ïïìRÜR?bŸ'gˆZÆ?`®
"nn?bŸ'gˆZÆ?ïÉ6­ïš‹?€Oب˭<?{d©£–®?€Oب˭<?ïìz/Nª¼?Iïÿ
x8?c…ÐóMÄ?Iïÿ
x8?ïðlÙ6‡?Wppw?_&MmƒR'?Wppw?ï½ÜAè`Z?…ã»…åû?€ˆïy1[£?…ã»…åû?ïÏ©ª)Ù?'#S/¬­?x+*ÒnÓÄ?'#S/¬­?ï«a­'??qüŽ"'?…'"ºè-?qüŽ"'AGN4FGL J1808.8+2419?êh	Y"–@3¼c¾ì9zÀ:Ïì""9À<XÕï‹=¶@ D›—ËŽ3@ð+[Î\ð?"J_Ÿ¢È?(BŒ;À?œ¼bØxÂ@1øûÔÍ!?ᅥ",˜¿ë…ë1;â.¿ÙÍî \+z¿è/V•8¿Ä FÜÞ<â¿Ý‰/žÔAGNbcu1RXS J180847.3+241923?ïû匔Öð?6rÚâ‹/?@iÍ2Ë4?6rÚâ‹/?ïåЍ\ۉ?~"µ {¨?j/r¥ä&˜?~"µ {¨?ïí8¿±}³?a¿­9gŠ?bÇ@<¤TÂ?a¿­9gŠ?ïûÕíe|?+ÉEwq?Cœ§VßZ?+ÉEwq?ïõ»°'%ÿ?Q}@–GÓr?Tˆž§yñÔ?Q}@–GÓr?ïš?2>z?'Ùن¶Á\?‰p3†Ï™Y?'Ùن¶Á\?ïØg(ò×<?zü'Ìhmç?sÌkœ'á¶?zü'Ìhmç?ïì!Cû
+?VoI£/ð?cÞ»Ûº…µ?VoI£/ðAGN4FGL J1808.8+3522?çªÛWÌg@7s²$ªÚ4À:ß\×qk}À<u¯§"Y@³ò ™R¢@EĚÏ#¿?щĄ©Èf?ÚPÓ!z¤@w|7‰?òI"Ž³°¿Àgّ×-?Ѩ¡ÿïŽï¿àx^졬¿à²öañŒ ¿è»ã?ÕÙ¿ïøbý¦3†AGNbll3FGL J1809.0+35172MASX J18084968+3520426?ï,¨¶En?žÀ9~le±?šjïЊ.?žÀ9~le±?àÔù
\>3?Ì[3"'~?ÞV
ëGƒš?Ì[3"'~?î9¼œ=A?œc™A)÷è?¬d>ꇮò?œc™A)÷è?âÕ6WÚ[?­¤ÛA.É?ÚU"QÎKI?­¤ÛA.É?ì/¦`ÒRÉ?¸ðØ;]&¶?¾'Ìùmi»?¸ðØ;]&¶?ÀtÇeV?ÁÁ5…ÚV?ëâÎ&œªy?ÁÁ5…ÚV?ë x?®"˸{;?þϗò?®"˸{;?¼¨šlÂò? lÑކ=?ìjì²g¾"? lÑކ=MIXED4FGL J1809.3+2042¿ï˜ë7µ¾@2Ao!öÊÍÀ:>Ï#¿!éÀ<VÇM1;@†Ò£¦bÖ@§—£öî?º£ÅA"¿w8uKï?¾]‹¡^_@Q
9òÑ?ï\6f¿½{B*8¿àŠUú˜{¿ã®bHŸ¿Ömt¢"?¿âG àö$ŠAGNbll3FGL J1809.4+2040RX J1809.3+2041?ïòDŒZ?R&MñÌGÙ?[wÊõƒ»'?R&MñÌGÙ?ïÚÙ3§;2?@oô¿?r"f11Û*?@oô¿?ïâox³Æ?hdj÷éZË?mëfOúC?hdj÷éZË?ïáñ¨å´?T­:þ0?nç_Y[®?T­:þ0?ï¸6H&ö?x€sm4Å?òn]l?x€sm4Å?ï^k—õ÷á?¦VxD?"2Œÿ‰5ê?¦VxD?ïÇ"îŽàÐ?ò`,×ù£?|nˆÇ­ß½?ò`,×ù£?磊#Ÿ?sÇÃtp¬œ?†¼^7X/?sÇÃtp¬œAGN4FGL J1809.7+2910?æñ·ëòµr@5EV:Ÿ8?À9ƒ-±éòxÀ;í.I¼â@ꊁù"×?ü3=D.-:?µ'‹>s>w?¹Æ]qö•@Xå>³™ö@YmÇXÅ?ïàCß銿å×Ù`.¿ÓcY%¯g¿×#¡šÄçÑ¿áa'·'I¿á€0q·ÓAAGNbll3FGL J1809.7+2909MG2 J180948+2910?ïý{ÐÓ9?,wÂ?4!x¨˜?,wÂ?ïÞ(Ï×ï?yZ»‹á?pë˜#Ö©"?yZ»‹á?ïê@VÙD?iyfÕ>cÓ?e¿î	³¶?iyfÕ>cÓ?ïÚÿIij?Qö\C;?r€[#w|?Qö\C;?ïû@®yƒ,?=
öHß&?BýF'%ë?=
öHß&?ïe•[
Š?£ÒÞ÷b?"M_J¹?£ÒÞ÷b?ïÈ×òð¢ë?€a(
mØ?{"¥ëm?€a(
mØ?ï•!4'7?q"9m"ïð?Š·¹okÖd?q"9m"ïðAGN4FGL J1810.7+5335?ï×l™Âo@;i_JsÀ:[Þây|À<'d}Xs@¸ŸJ;?þ¸\'·ÕÅ?ÂÜýŸ?º>—ãåî?ùž˜5@ "ô>?ëf?úìÆ¿æ‹vÁ¿ã±MëE]Ø¿Ñ¥øã?ì¿ãÃ?»òn¿áAÝ¥¸AGNbll3FGL J1810.7+53352MASS J18103800+5335016?ïû¬':¾~?3œ·Õ‹ÿî?AM÷Û|Cv?3œ·Õ‹ÿî?ïìJf€?hÈ²ÌÙ?cú¶5ç?hÈ²ÌÙ?ïò|"2Ò?e–"¦ú£õ?[è…#»¨?e–"¦ú£õ?ï¢uFÑY?e…é^–"?‡b®pÍ9Þ?e…é^–"?ïõO!r¸Ò?PTր¢e?Ua¼Í—L?PTր¢e?ï±UDwu¥?ƒ·Ëêí?ƒª®×ÓÂß?ƒ·Ëêí?ïñE¤ÇA•?m˜16ô%ß?]t¶*ö‰?m˜16ô%ß?î‹9Òè"q?‰iȘ !ý?§Lbԍè?‰iȘ !ýAGN4FGL J1811.0+1608?åËóW"Ö*@0ٜ¾èÀ:UáE)Õ¼À<7tm&S@ •R&é?ÿaýKÙÆ?ÄTPåÔÝ?À¾õHÁå¾?üŠ=Ü¡@
ÐÏ֗{Ý?é?÷!	:¿ékÞuk¼ç¿Ý¡ ñ§£¿ÐúBœÜ=¿çÎ8§ç:6¿å´ ÓʘAGNbll3FGL J1810.8+160987GB 180835.5+160714?ïý"ÊÞÇ1?'À@»"à×?3a¨MÂ<'?'À@»"à×?ïÒs^‹?~?kO@Dg³?vÆP¢Rý]?kO@Dg³?ïò™ýá?Zå¼%>b?Z̸¼îŠ?Zå¼%>b?ïô˜¡Þç?;¦½Ú%ç?Vμ±¹°l?;¦½Ú%ç?ïø¾Š?I¥-ÚýŠ?M‰½Ù\?I¥-ÚýŠ?îêÝ«¹¤?¬¼ÇæÆäz?¡R%AÒ	,?¬¼ÇæÆäz?ïÕ¨á$?€{Úê»V?uz¬ïEø?€{Úê»V?ïâ
9~?XÕcs먼?mõüº†ê7?XÕcs먼AGN4FGL J1811.2-2759¿ìT˜ÝÿF"À£D^Ô¡­À9ðb¿¤À;¦Ù>Ëê@ r%|ç1R@
òœj.r?ÁÅ[¿Cw?£P»¯C$?æòûE•‹@–šÆÀCR?ïI¤^ïz¿å¸ýÿÚ¿åìŸÀÐU¿Òõ¦n"2¿ä›…AÚ¿Û``="(AGNbcuNVSS J181120-275946?ïêë9…˜í?p—‡¥ˆ?eÆ­AJÝ?p—‡¥ˆ?ï­ò4Ìv¢?šÅjTrù?"ƒr"ƒ˜?šÅjTrù?ï€lor‡:?'p¼A9Ò?ää0%¯?'p¼A9Ò?ïÑÃà¦.º?Zž3Y68´?wÇ«?Zž3Y68´?ïϮ݉ġ?hT"¾ú}?x('6þ'»?hT"¾ú}?íü•ùb=?ÀÕîê.¤?³€Qì¼?ÀÕîê.¤?îèÈՂ?÷ÝòŽþ5?¡~"vóZ?÷ÝòŽþ5?ï#bUéE?†"x?›"µBÜ7h?†"xAGN4FGL J1811.3+0340?ï3ªXrv¯@%4¢v·íBÀ9-Ôx'¸ÕÀ;®n@O{h@ßqÎ#Žû?û±ëºÎ‡?±zƒ(éÙ"?¹£Íúõ)7@2‰¥/ÏÑ@ ý+¿ïÿýFKê?ïÿàU?Íu¿Ô¼Q?Û0¿×a!§¼r¿ß
®ñð¿Ýî–áƒh*AGNbll3FGL J1811.2+0340NVSS J181118+034113?ïý3Ðo¢-?1¯Þ梗?6a|"#?1¯Þ梗?ïuÄ߇S`?šá¬<e_K?'Gd"?šá¬<e_K?ï…arX/?%^~þr=?Ž¹§±(dJ?%^~þr=?ïØ0õٔ?W÷—Øϒ?sçö'qÍè?W÷—Øϒ?ïû[‹AB?@þ_–n@Ø?B'Òk±¾?@þ_–n@Ø?즆¨ñ€?ƒû"'˜Á?ºËÊ¿èt?ƒû"'˜Á?¾cŸ?‹—–àÜ?ŠÜ'FPM?‹—–àÜ?ïx$5X@M?<tLp'‡?ûy]Žü]?<tLp'‡AGN4FGL J1812.9+4249?àyàN3ê"@8ÅAt>–>À:–´ -œñÀ<g&••þÚ@¶-÷ `@s¤<ŠÊÊ?Âù©d<ën?£ªËñº?ß)í9SÞ¤@q‰¢¬=?ŒUe­È"¿çÏ d#–¿ç(9À.e¿çê	*v¿äµ`iÍ#4¿ïÿäâBTäAGNbcuNVSS J181308+424853?ïû|a"3m?=wÞÊ_@Ö?Bz¿SZx?=wÞÊ_@Ö?ïðÿ•ˆ#6?b,¹Ñeç?^Ôe?b,¹Ñeç?ïíí‰þ?asêkïÁ\?bêSs'?asêkïÁ\?ïíÄF@%?F‰Ñ"ÖâÈ?b;¹…ÅkÍ?F‰Ñ"ÖâÈ?ïø±Ä!œL?JØ6ê?M8ð"½<\?JØ6ê?ïºa÷ì¶?ˆ`îâ‰=$?{ç"lŒt?ˆ`îâ‰=$?ïá{]Ìíb?o¹Æ\^e?n"¢aÍN?o¹Æ\^e?ïÚÉ9ÅI?vüÔ|n?Œ	M `¡ð?vüÔ|nAGN4FGL J1813.5+3144¿àø¶á7Ò@5`RÚšÀ93®üm¾À;Êù²Þäý@çƒzú@E"FK=ì?¯‰ðÚB[?¢èׁÜ9?ôÌF嗞î@
KH¨»J™?ïñè°X"¿åT}e†l–¿Ýs>#§$¿äloàŋ¿à—¦°'«¿åbf'P¢AGNbll3FGL J1813.6+3143B2 1811+31?ïûÒeàQ?5 A¤igT?@¶gqçH`?5 A¤igT?ï톞ȶ?jH;Ž¦ä?byaÕç?jH;Ž¦ä?ïà<Q¹í?yG@EgU¶?oÃùqÌó"?yG@EgU¶?ïë>)'ãì?PZ|Ø€s?dÁÖ¥AÜ,?PZ|Ø€s?ïî"î*¯?Z^å#<éh?aùzù Ý?Z^å#<éh?ï·ÓÜ¿Õ?‡x÷dÿH?'ÉœÄ?‡x÷dÿH?ï×uŸ`ÐG?|¸JL'õM?tE0X†Ø?|¸JL'õM?ïËÜ[
N?f…W)g™?zþçÈlé?f…W)g™AGN4FGL J1813.6+0614¿î[bIKM†@&xžÛø¹»À9…È•/§À;Û$
¡C²@kىô‹?ýñ ¦ÔÀ?¶•ÄÞýã?ÅyÞonM@¡ÃA2Ð7@	H€ô1?¾¿·ë˜iî±#?ƘŠ:N¿Ô>ðÁ¿ݏO(\?œ¿ä}Ëùï¿çK`6÷cAGNbll3FGL J1813.6+0614TXS 1811+062?ï½N/–y1?©"´­=²µ?€¬tҏ·?©"´­=²µ?îméæÊ5)?²H®ÍL?©!a•ðbk?²H®ÍL?ï'jB‹b?ŠÖ•ÌhŠ?
Ò°Ï[Á?ŠÖ•ÌhŠ?ï7õÇÒA?qÆôޔA?™G$m!à?qÆôޔA?ï@'™¢ÓÕ?™LøÀÁ\É?—ï¬Ë¥…`?™LøÀÁ\É?ç<èa0z$?άk6Š?ц/=Ÿ¸?άk6Š?ífì¬ÕÂ?¥{V!DªF?´Èš ñê?¥{V!DªF?ìëþHùL?Ÿˆq>‹ÊÝ?¿h 
¸5¢?Ÿˆq>‹ÊÝAGN4FGL J1814.0+3828¿î•;àÆ@7dÝDUÀ;l$ˆþÀ<¤$u*Nˆ@Ùܪ»U@!€[2•?Ãé•Zo¸?€ËŠ#ý,³?ÁQ׎â@…DM÷?ï˗C¿äª¶ÂŸLa¿èo,s%'Š¿×j,#tyO¿Þž^då1ó¿ë/…>BÛÈAGNbll2MASS J18140339+3828107?ïþm–K9?f!¢@ú?)'æÇGnS?f!¢@ú?ïóI5å%?b§éä@Ï?Yïmµ1ôó?b§éä@Ï?ïöøx¥?[+­imt}?Rå	}Vì?[+­imt}?ïûCrñd?(Ö·Ë?Cšó¼Çº?(Ö·Ë?ïü¤˜üÛ?5ÉÅþFæ?:Û9á4h¤?5ÉÅþFæ?ユÚûÂ6?†hsÜƔú?€Z‰E†ðf?†hsÜƔú?ïò'}žïÍ?i–VñíX?ZÝÕ^5$?i–VñíX?ïíX·ÀåÓ?R@f|ª®;?b§H^¶•8?R@f|ª®;AGN4FGL J1814.2+4114?ê£C{w<@8 9GIj­À;²_c<æÀ<…"f+®@ßÁ_±@@h–<"?ÍøU¼ ì?¿ó¬-AØ?ð+uϏö@Wâko°?îQ6ßD—¿ÝÔäžO¶Í¿è08­¿è´" [Tº¿ä2ÙaÒ£¿ïÿð`OËðAGNfsrqB3 1812+412?ïþµ)dtÁ? ¤~}ÿÔþ?$­m‹D©j? ¤~}ÿÔþ?ïïøäòž?aî!=ä?`␁¹?aî!=ä?ïëôý¡	?e¤ež-p?dî
ÇE¯¦?e¤ež-p?ïëdàÝÙm?EñƉ@Jé?d›D'ª¯?EñƉ@Jé?ïýÏXd½f?0UOÉ\!?1…;¼5O>?0UOÉ\!?ï¹	ËŠ?…÷–Y[,?½¾VÝEb?…÷–Y[,?ïÀJ8ïpø?€Õ'»€~}?Úãœå+þ?€Õ'»€~}?ï†Tú"?xû/tV{?ŽjÁpÌfŽ?xû/tV{AGN4FGL J1814.4+2953?î?—Ï·ZA@4¹à`þHÀ:œÁr%·À<1ýKÙÆ@¹‹cÅ@EI@»²?Ņa(c÷K?³ÄÓÚGó?ìö®G¦‡¿@
è§á6¼¿èIžŽ‹t¿á< B¿çÄä þé¿æô,Ý®œ`¿äª$+X¿ïÿ6a;aAGNfsrqB2 1811+29?ïýàÕ9¥?-y^¡¹ì?0ÿðQD'?-y^¡¹ì?ïí"V«!E?fš%)ãÝ?b{©e\Ú°?fš%)ãÝ?ïé
-‰Ñ?kS®ppÌ`?fõÒrݦç?kS®ppÌ`?ïû[u>?*И>è?B'+6øÍ?*И>è?ïüPjs×?AS¯;üÚ?=|ªüê‹?AS¯;üÚ?ï¢zøEn?'Cu§p?‡aX~Š?'Cu§p?ï­§pŠà?‡ñfQq y?"–>±›·å?‡ñfQq y?ïâ$·¼¼¬?^kbw?mÛH%Äp?^kbwAGN4FGL J1815.2-2715¿‡¤šXÐ3†À_óÂîÀ9f}å,õÀ;7sx @=ϕÿÜ@®ï¼»Ý'?Ã_À‡'?Äÿ{á!îg@±ÕÝ톁@~žHªé£?ـR`J¦?íØRÂD³Ž¿åþ‹÷§q¿âÊ¡yaë­¿ç&r@T"¿ìÔ(᠙hAGNbcuNVSS J181510-271304?íí3¿A–E?Äï 3Ò?°–baAY?Äï 3Ò?äIÿû£Nú?ÏÐʎÀ2ò?×l¹b?ÏÐʎÀ2ò?íyº¿ë#5?¦¢Ý籒z?´2)ÿÊÿW?¦¢Ý籒z?çÛ;ÀJˆd?®9¼¿W|?ÐIˆjï7?®9¼¿W|?ä­r]?̲¯zã?Ö¥ÇÝEù?̲¯zã?ÍØaH¢ä¥?ж›)‰?è‰ç­×F×?ж›)‰?äEԍ,ñ?»¼'+í!?×tVå¦È?»¼'+í!?ÈAŒðÇ?´Ç?—ù'?éûx¯œÃÎ?´Ç?—ù'MIXED4FGL J1816.9-4942?ÙZã°ÿ£À.U¾'bEÀ9¡ÑÒÆÀ;ðH±I¹‡@mÇ՗ Ã@ôÉBԐæ?¶Í¬½?Æ®÷ϯÖ@Ðì1"@\ÁÂ,µÁ?ïøè^£¤_¿ã´¼j~ùÛ¿âqÚ}ºjõ¿çƒüÿšs¿éâ@!-L>¿äÔê"H)dAGNfsrq3FGL J1816.9-4944PMN J1816-4943?ïÖq""9?šuœ&v=G?t÷Çc·†?šuœ&v=G?ïígnp˜f?rŽâ<ë?b˜'`¬êb?rŽâ<ë?t\Yƒ?ƒ´Õ2ïô?ŒbޚË5?ƒ´Õ2ïô?ïúüõÖÓ®?+¢²ýýï??D)&oSE?+¢²ýýï??ï¶ÄdjÛ
?ám÷2¼?'NæòWÀÅ?ám÷2¼?ï·¡"1GB?˜òy²Ã
?'šëo?˜òy²Ã
?ìËBI¯)?ª®C+Æ#Þ?¹§=í²†·?ª®C+Æ#Þ?ïëÏã=ã¢?Q󬨰?d0Â^t?Q󬨰AGN4FGL J1818.6+0903?înt´ È;@&¸÷QÕÀ9S€éŸkkÀ;¨J¶Ýw@÷—´&¹@#z›§Ó?µ8ð6‰T?ò	½n
@
Jè[žŒ@(2Oˆ~i?ÔÒ«3=¿ÜºÂÇ;=¿å?çÁŲ§¿å{C؜䨿èeçPÑÑ¿ïÿ5Õ¤â£AGNfsrq3FGL J1818.6+0903MG1 J181841+0903?ïd‹A+Y?¿fŒ*_ú?"n—Þ°Ë?¿fŒ*_ú?ﵩ*cßV?°
Ñ¢\?'•µiÇÚv?°
Ñ¢\?ïª4Ó,ž€?}ÌÞêÏ?…rË8Gü
?}ÌÞêÏ?ïõaHÝ??:ÉÑbùÜ?U=oeSAø?:ÉÑbùÜ?ï†ø¢ò‡?%ÉöÖ!?ŽA×5½nc?%ÉöÖ!?í£5ïG˜g?À>Keë''?²æP†Ÿ#Ä?À>Keë''?í÷9Š<N?¡®.‹Š‹?°F3ª¢6"?¡®.‹Š‹?ï×dÈNg?``—oÊʈ?tM›ÐÐo?``—oÊʈAGN4FGL J1819.1+2133?ÚM\ù™ù*@0~ýX…ÓÀ:P-zŒŽÀ<L|tÅ¥@í	Yp	@tw·?ÀɤyF'á?ŒkÕÄ ¶ø?ϵwß?øüyzë-¶?òÉâ¿è,YÅn3º¿çe`¬é¿ÊU?øh†ý¿Úð®=ës¿ê¨U¿O5ÈAGNbll3FGL J1819.1+2134MG2 J181902+2132?ïôØ1Yê,?N¬u«%?VOœÂ»Hb?N¬u«%?ïÂmiSÅ?'÷RŽ¦`?~õIA·5Y?'÷RŽ¦`?ïâ(C–ß?o:y½J¶?m×¼&¥Èß?o:y½J¶?ï«Âø?h¶ÝnOÿË?…8ù¾îÂ?h¶ÝnOÿË?ïå]›,?dø1îzG ?jí¢ûƒ»?dø1îzG ?ïÍ¥S¥Þ?¦Ã\ñW"?ž†KU‹D9?¦Ã\ñW"?ïÉ;Óô<?'F?7¡û?{braw?'F?7¡û?îÁqàÿ?÷¤¢óEÄ?§ãèހrd?÷¤¢óEÄAGN4FGL J1820.3+3624?ÞÖRè/SÖ@5Þzt:À:"Y~À<ƒÎod;ê@ èíˇ'?ü5ˆ]13?ÂêÄ.˜š?§%E<}½N?轶ÿÛíÒ@½rã¢QN?ïêÒa6PÊ¿éV!IÑ°¿áãп "`¿Ê"~èx~¿ÑÐrß­*¿ßlg1gAGNbll3FGL J1820.3+3625NVSS J182021+362343?ïýXÚ©?#¾°¥Æù?5;zg±Ò?#¾°¥Æù?ïÛõ'?eµ'ïìl'?ao[3(µ¥?eµ'ïìl'?ïö·È6m®?`ÞÜ	yÓ?Ro"$¤>?`ÞÜ	yÓ?ïôŒBTI•?:´u""?Vç{+q×4?:´u""?ïûĬ—Î?5VRR™‰X?@íMˆ—C&?5VRR™‰X?ï³ñ'[Iä?‹Äö¤—¨?ƒ¶†½?‹Äö¤—¨?ïúlµ,i?Q´é¾	p?FM*JÝ´k?Q´é¾	p?ïßrã‰õ?]$×à`W?pF·—*r?]$×à`WAGN4FGL J1821.6+6819¿Ýâ]xAÄ@;Ìú¬Ùè>À9<f0¶1À<"øR@{ó&þœ~@—AЄè?«'ÈûîÃ?ªâðz¦å?÷ÀW xF@9Ê&)?ª
‹ýáB¿çö!ãÕ}¿çÛÓ/½\í¿ècúÿæ¿ëÑT†jí¿ïó'^±ŽAGNbcu7C 1822+6816?ïýônô¡Ê?"eR½Vç?0\‰@½ò?"eR½Vç?ïö<a§‡:?WŸFbµk?S‡<S|+°?WŸFbµk?ïç±oy4Ÿ?eå÷¶w?hNÇdb?eå÷¶w?ïüäÇë;£?., 'm:¡?8ÙÂ$Ä4Ÿ?., 'm:¡?ïþÖ1ù'?{"HÓU?"œð$6‰^?{"HÓU?ïÕd!¬fë?zCù}ÿ?uMïî'Ô?zCù}ÿ?ïææօªœ?lq3šŒ±?i)`8\b?lq3šŒ±?ïø΀?C>ºêñÄ?Oç¯÷fP?C>ºêñÄAGN4FGL J1822.0+1600?ïz't}'@+0Ãóà7
À9úmû†¼À;ä$>úè@‹hÓ©@2¼›&b?ßàŽ¾?ÁjýyèÏ7?ø¥=§*{Õ@(",J
æ¿É]q¾‰¿æ@³^'°Â¿åJ*Æ}'s¿ìÿGþò8í¿ÑfKÄ#°ß¿ïï©:÷LÓAGNbcuOU 134?ïù<2ÜÄ?J€4Sºeö?Kô(¤cÃ?J€4Sºeö?ï¾Ä«û?"lXØÞ"?€NÕFâL?"lXØÞ"?ïÀ
6´?~=áÏø­$?úä­'6Ä?~=áÏø­$?ïâé4ȚÊ?TÉ8/?mËkŸE‹?TÉ8/?ï¯hSâ'k?a[<í?"%뢗?a[<í?î'){'
?±—àŒ~EY?§ÝhI—-?±—àŒ~EY?íÙ]¸S)Y?¤ZÈÅÎx?±5>Bœ7?¤ZÈÅÎx?îè̤!̝?'Ý8T?¡s5½O-?'Ý8TAGN4FGL J1823.3-3720¿Â««KëmÀ%íîÇÉXÀ:Î/OxäÀ<‹Fí$[)@@nå»Ü@Ô@C¼î2?Ôæ|+õ|?ïÿø]Ê5™@Ç%Þ¶Ú@›ëƒq9(?ïà7]d_%?èïÕ¿èÀc'†W¿ïþ.~Ãq?ïYِ)®O¿ï¦€g™lMAGNbcuPMN J1823-3724?é	X'x-Ó?Î2ØbŠÂD?ËڟbH´?Î2ØbŠÂD?ì"ª\_|g?ÅÑpϺ¬©?¾ê­Å?ÅÑpϺ¬©?çúB£'?°*£h`¢¾?Ðz¹üÝÙ?°*£h`¢¾?ïÈQlqT?ßÕØo.?{×{Õv(?ßÕØo.?뻺'Ž?ÈAäp't?ÁÝõÇ ?ÈAäp't?ÕÌo4@Nz?Ô8ÈjÈ)?åÈeßØÃ?Ô8ÈjÈ)?á¥Â8Zv?½{ÀÉ;ü8?ܵú{K?½{ÀÉ;ü8?êê•ÇÊPé?ÃcÌÖæ^Í?ÄU¨àÖ¼\?ÃcÌÖæ^ÍMIXED4FGL J1823.5+6858?Ð	`'x#c@;«h¾/{À:(ðzPþöÀ<oE§©ý•@vb)?êQ?ÿ…C5ßµÞ?¹Ãy'çI?Ðît1Žî@«>o§X?ûê"Ò/¿ï@)æÙ?ݤQ¦ùT¿àþ3ÂOEc¿Þæþ¼³úï¿ëüYýÍJÌ¿ïÿùµc#¼AGNbll3FGL J1823.4+68577C 1823+6856?Û
ù"îú?ÉF­¹a5$?âzÿƒ6ƒ?ÉF­¹a5$?Ûj"Ú?Æ߬߂Ã%?âJð=·'ö?Æ߬߂Ã%?âFËZJ¾?´ˆÒðÿç>?ÛûriKj"?´ˆÒðÿç>?âÒ}!$#?°2—ÄÅ÷?ÛÊ[½·º?°2—ÄÅ÷?žB¨˜¦Yº?—8¤§¸Âß?ï
ê»d'?—8¤§¸Âß?¶ºCŽ¡?¹…ùåve?í(·ž‰ºÌ?¹…ùåve?»Âos!Ø?¦Ö @cÞ§?쇲›Äþ?¦Ö @cÞ§?µ†ÑËå?¡vŒÃ*3F?íO?eƃ]?¡vŒÃ*3FMIXED4FGL J1823.6-3453?ëwé܅°À#ß6ï€UüÀ8¦}¢ÃÀ;~ð=ë@ça•q@à?û(œ6,ø?§}–¦B¹?«ß¤jØæá@+Còž@û´^kñ?ç$çá¦?ïù—02ͳ¿Ö[œ¾'!€¿ÒŽ"&±¿à_ZοԪÂ@ÆAGNbcu3FGL J1823.6-3453NVSS J182338-345412?ïÿD³… `?>CM©?i–á°Ô™?>CM©?ïÞ£w?€U2˜uێ?p®÷à`x?€U2˜uێ?ï‰Zéý×~?'—ÖŠÒw?©Eƒù¼r?'—ÖŠÒw?ïéíÚìþ¤?V§¾b‹Ae?f%¢Ãþ?V§¾b‹Ae?ïþº¸®Ê?&•f"UD?$T€äýÍn?&•f"UD?ï!Çîk­ù?®àí5åúw?›Ç7±ªÚ?®àí5åúw?ïxÔh*>v?"+c¹–m?årõÇU?"+c¹–m?ïÒò–¾{"?k¾y?Œ}ì?v†´™ã?k¾y?Œ}ìAGN4FGL J1824.1+5651¿ã<ߘ<³v@:Ù#d»À8w–Б}kÀ;ÛLg"t@½vá³¹«@o	R
?žöÐ"äþ¿?°'²o~h@§Ó[\G)@k#Bû'S?Ë%=|7^¿ãT"Ö¿å¿ž ß¿åÚÛo›ï¿ç!ueݪk¿å#slß&lAGNbll3FGL J1824.2+56494C +56.27?ïý{Êëe?)yÈi?4!¨"YÎÞ?)yÈi?ïñ÷9e"ó?`7øQ!f?\¥©J!?`7øQ!f?ï阡]S?f:œæ'Žç?fg_
€¥@?f:œæ'Žç?ïù›	•"?8ãÛrJ?I'Ä©z?)?8ãÛrJ?ïþ9¾šô?&DևЀ?,d -û?&DևЀ?ïÎqY"tä?|6–#÷6?xÇSxdv?|6–#÷6?ïìÅ=®¯?o¨08i—?cø:ýj™
?o¨08i—?ïîÂV\ê?R'Ž×úux?a=üÔ>=£?R'Ž×úuxAGN4FGL J1824.5+0107?ëìâ8fE@ÃX¯Ä~À8äB(™|=À;	‰H¾I@.<<œ=Ž@.—eóS?¸Ôž}Y&?²+
Ò&?ô~žš@*êëñ«)?ê¯+ie¿åù	p¿ëgV@S'3¿âT	×ð~¿ë^*Ã") ¿ß&a"˜ÏAGNbcuPMN J1824+0104?ïòńÙîô?UIÕ)qLK?ZtöéGÚ?UIÕ)qLK?ï'çü‡r?Ÿä¿»Iö!?‹F8½n‡ˆ?Ÿä¿»Iö!?îçV	Kà?—ìŠ(Vn?¡ŠŸl÷?—ìŠ(Vn?ï׋pû¯}?Yê-(TÏd?t:Gs	ù…?Yê-(TÏd?ï4µ·1…?›~g¯F?™iI>úô?›~g¯F?í{y\|ž?½"Ò¨Œ";?´$5ÕH?½"Ò¨Œ";?îoüe¹?Ÿýf3ô<?© ;\=?Ÿýf3ô<?ﺺÊ0?†ãg2ã?¼´?†ãg2ãAGN4FGL J1824.5+4311¿Üý³0æÊ@6ׅ@FA-À:Ô{bvíÀ<+¼FlÌ@!4Ö½;ŠE?ûÇ(-E³h?ÇWOGß=?´àú@ÎQ\?ð܆Ô@Í:Ó»~q¿è¿!Í°"¿¢I÷<Ynÿ¿æò•^KË¿ß!š•m¿É¦hßè]w¿ã•õôVÿAGNbcu3FGL J1824.4+4310RX J1824.2+4309?ïþB0èU?5ª•.…%?+Þ+}Ø!P?5ª•.…%?ïìûñ,?li‰%ï?céùÍC½?li‰%ï?ïò ¸ÿ‡×?Xs("'Tq?[¾Ž,àó?Xs("'Tq?ïîÔÏá»?G²y(þ?aî+8]T?G²y(þ?ïüË<KW9?5dŽ½fy‰?9¦
ê½?5dŽ½fy‰?ïªZ@µŸ+?‹_œ4ãéG?…ioàV¥%?‹_œ4ãéG?ïôBDs!‹?^aúñÎ9	?W{vÒE
å?^aúñÎ9	?ï¡éÉ ´š?zv+Ÿ¥Ö?‡…»Buk?zv+Ÿ¥ÖAGN4FGL J1824.7-3243?ç<"—Ì1iÀ"V,UÉ`1À:­_ö	ÜùÀ<"Ó~—¶@?8Aºàf@O8œÿ¨?ь®¤˜¦*?Ùk¯#c²@	ŒªZ±ý>@Ùúf=!?ïʇ½ùö&?âtÒò¿â.ÂöŠ5y¿âcò¸ï 6¿ïôcê‹#µ?ïj¾º»RAGNagnPKS 1821-327?ìÞ\椩?¿©Ïùö"?¹
È´öS?¿©Ïùö"?è9ó
Ô)
?Ëž×ÆûÒ?Ï3ȯ[Î?Ëž×ÆûÒ?ëB*m£Þ?§¯ËvjÓN?Â÷VIsø†?§¯ËvjÓN?ê›PWJ-?©–
–=/?Œ¾¢×IÂ?©–
–=/?éS³Ò§È?Ë/øý="?ʱ0·á`á?Ë/øý="?§În?ÇÐÏP_¾×?ëVzüdY?ÇÐÏP_¾×?âCF³–â?½û)}8 >?Ûyr™òÒ<?½û)}8 >?ÏçñxJ5ü?¹"á'@?è¡ír?¹"á'@MIXED4FGL J1825.1-5231¿ïn¨ö¦1À1u;÷'À9N\(õÃÀ;ä(ôëÐ@_êVËhÊ@;šû™hò?°Ù·µä?ÀªqK´´@Òµþ,Á@'dkåV?qÏJ*›Š¿ÙÀ.XØß*¿æ¸÷˜Rq½¿ãõՅØò¿êC7¢®–+¿ïÿ ºöAGNbcu3FGL J1825.2-5230PKS 1821-525?ïøÐH­Bï?DíO:Ÿ'e?L¾ÜÅ]_?DíO:Ÿ'e?ïòŸvþ9?c{&ÿ(®?[öÀ±Î~/?c{&ÿ(®?ïÃM¢u5a?w5Äøfß?~Y.©èo‹?w5Äøfß?ïÿd¼Ãg?;Õø
Ë?hep?;Õø
Ë?ïî'$«í?\NõfÍS?a}í¯Y)?\NõfÍS?ïÈò4å?ˆ0¦ÈYµ?{†æ\ç"?ˆ0¦ÈYµ?ï=6å¢å%?'P"L·[?˜Y#PÊÅL?'P"L·[?ïþE"Òpƒ?!kŽ8Ú°?+­ÒµÈ—Ç?!kŽ8Ú°AGN4FGL J1826.0-5037?ÁÑüfsÒÀ0Ý\…<ƒÀ:åCä/À<LERðh@ %ZÕHœ?ý͘T<?ËÏ?tN†?Çó(ªB?ýÒK&nÿ'@ݺÄâr¦¿ïþM"r›©?ïÿöÅĚϿ¬&SUȬ¿ÞøC¾EËf¿ç]þÈs¢¿Ñ‡wã¼RAGNbcuSUMSS J182551-503914?ïû…'ØÈ??L'Íʬ…?Aë`ÿGD?L'Íʬ…?ïà'…Þ"c?z"MÕ:w?oØyÿ…V?z"MÕ:w?ïÁ©ÿ Ç?€©2j¬`?+e©È©?€©2j¬`?ïÖë|:c(?YQnâRÇU?tŠAë½gÒ?YQnâRÇU?ïö@CðxV?P -ÿÅ?SxŠC#
?P -ÿÅ?ï™ßɘ~«?¤‡=«Å?‰ˆ
–p¹3?¤‡=«Å?ïmNî-MI?š-@¿ˆ£?'V"3wò?š-@¿ˆ£?ïG÷Ô0?ƒò¯i2?—A µò?ƒò¯i2AGN4FGL J1827.5+2015?|›êΝa@,X–Ý&·$À:ãAÒ2g[À<K§°³''@ N+9>ºü@	T!ÀD(?Ãߥ+Ï¿¥ú—$82e?ã|‰ˆª^
?û9ÐUîI?ïü!ƒÞFr¿å(Gýo¬á¿ãœa?`9¿ÚÑR+Sk¿Ñxâií¿íC·'sAGNbcuNVSS J182730+201309?ï÷NJ¡6Ï?NÚ­‹§]?PpêÐÐ0ê?NÚ­‹§]?ï¿sèb³?†ÁPz"Zj?€:b÷x÷R?†ÁPz"Zj?ïÅAîëcC?€`÷"¡°?}_¤kf?€`÷"¡°?ïÖFÎpâ?YŒÿ:ˆy?tܘØ5¯?YŒÿ:ˆy?ï暥w@?d3{®}P–?ieZÆÌ·ç?d3{®}P–?î–çëŒ*›?®ÍJÿ‹Cž?¦'BñÓS?®ÍJÿ‹Cž?ï"¦jŽ?ŽêÉ­ œ?‹9Öl\k?ŽêÉ­ œ?îÏ•ŽG+?'Y±G\;?£¶¦?¦P?'Y±G\;AGN4FGL J1827.6-4029¿ÛY§ï¦I3À*Q´þzÀ:Ås½fþ<À<Nx"PŒà@Q†QŒ@njCoÁY?ÐP¼›|GÏ?ÝaÅÂÂ\Ü@
•"äþòº@Xâš>…?ïùu'
5ô¿çumjf¦'¿Önà2…8¿îoÝÞm¿éÏÅÀi<¿ïÿ®¡hšôAGNbcu1RXS J182724.8-402904?ïy›'˧¼?'æ,DVœ?Ì¦‹v?'æ,DVœ?îB†|L?®&Λºù>?«×žI%U?®&Λºù>?퇌ÒÇô²?ŸHáÄvT*?³Ã™iÀZp?ŸHáÄvT*?î¤=k½µ¥?‡‰®«SÊ:?¥¼)EÜs­?‡‰®«SÊ:?íۗq\tÜ?µ0ޅŒ{?±#DuŠLž?µ0ޅŒ{?㛪"3½?ÐÝìWµ&F?ØȪ÷˜…ü?ÐÝìWµ&F?æ"Tà¤gu?¹¿A«hp?Ò×V>·1?¹¿A«hp?æ¯ÃfÐ?·ËKÒÃ?ÓÚ¡öy2`?·ËKÒÃAGN4FGL J1828.0+2634¿É덣
®@0ŽØ
±À;­î»4À<Žä†&ö@ ¬!®{}û?þ»ë¹!^?Ð ‰ãC0×?É87)Þ?ønã]2
>@¡€\[˃¿ïþR¡ªˆ?ïãë¸J_¿À®ŒDòMe¿áp ßs˜~¿Õj\|ؙ¿ë§A"4ØAGNbcuNVSS J182756+263313?ïאn¼e?¬snÿÀ~±?t7ÈÀ¹ô!?¬snÿÀ~±?ï¯EÔ[ȏ?"mDÕ[·m?".Šùãò0?"mDÕ[·m?ï¡5(o¤—?‡Nµtà_x?‡²µäÚ&?‡Nµtà_x?ï¿¿KK?dÝpTì?€=¥ëO?dÝpTì?ïÔCÄÙkõ?r·U,m"?uÞ§7ÁR?r·U,m"?î<:êrá/?¹¢A¬?¬<QV>8?¹¢A¬?ïH0#?˜¾…BfÛ@?žîVøCÏâ?˜¾…BfÛ@?î¾0Ò'L?"ÿ:›?¤òÛÓp˜?"ÿ:›AGN4FGL J1828.7+3230¿ã&wÊ@2Ÿl‹C•À: jüÎÀ<§Iˆà
ò@Í+4Ja?þyŒcP1q?ʜuìì'?äk•ð]Ì@–fœí@`Fë¡Ï?îé}'Ô?¯ ®ˏ¿Ö;™Ƚɿä…Lò!¿ïÿþó…õ?ïGÉÃ-ÚAGNbcu3FGL J1829.2+3229B2 1826+32D?Ñåv
Ž?Ð
5º™eå?ç
Dú¹w¹?Ð
5º™eå?ÞƘÁ?ТÐ÷¡.0?àœü3±w ?ТÐ÷¡.0?Ø¥c5sC2?³IÍû"ï?ã­NeF^g?³IÍû"ï?èÓo'M?±ûº¯'›1?τ³æCbÎ?±ûº¯'›1?Şg\j~?Å®â8_?ê˜f?håa?Å®â8_?µË`‹çò?½Éä`Î],?í_¦"Ó"?½Éä`Î],?Í`Â右´?³pø9ìN?è§ÏFœ?³pø9ìN?Ë£Òç‡Òá?·…•Ü™Ë"?éFH?·…•Ü™Ë"MIXED4FGL J1829.0-2417¿é©Æx'¦Àäœ@=òÀ9M	1´®À;™Þ˜§+S@˜#wÔM@´¶býü?³ÒŸt¤í‹?"³n#kŒb?á Ϟ8dË@¼‰¿±Ü1¿åŸ'•¿†¿Ú##´e"¿ãhÆ]Gô¿à6U\Rç.¿êŒÕ€Ðtø¿š ½R¡ÛAGNbll3FGL J1828.9-24171RXS J182853.8-241746?ïãRŸ¬z"?uŒmèäü?l­`eccª?uŒmèäü?ï½6ËTbê?úc, û?€²Mˆ­–?úc, û?ï•P/~ƒû?ˆãwœ	Y?Š«ô#ΝO?ˆãwœ	Y?ïÒ9«R6?d²‰
ri?vã*;¥¹?d²‰
ri?î³æå…^?¤OSO]`?¤Á'©aíï?¤OSO]`?î4sÇob0?·H»¶ž
ý?¬¸Ã‰	Ý?·H»¶ž
ý?î4$x–zç? 'lºV?¬½¸xP‡? 'lºV?ïE®Ûþ¡?‰³Ífç?—J$…S8"?‰³ÍfçAGN4FGL J1829.1+2729?æ}®K"­@0²{åS¬OÀ9ÄP¡C§À<L¥ËD@Ð<Q¿æ4@"îV,\?¼MfÿØ+¿?Äj´iS«¤@¦Ôš÷g«@ã·Shݺ?–tP›	Aƒ¿æ|š…R¿äñržƒ
f¿é¢>Çç¿ïÿ#–Ýýw¿ïúÚâ9EœAGNbcu3FGL J1829.2+273187GB 182712.0+272717?ïÍöûÊf@?©`¦Âý?y'6I¿Ç?©`¦Âý?ïm}ÕK
? Þ¨v¬/?'PEYÿº[? Þ¨v¬/?ïª0Ít´Õ?Ç€7=óò?…s̕ZÈ?Ç€7=óò?î²[x)e?‹ÈJ*G\?¤ßúKí«?‹ÈJ*G\?ëJá-_'?Àý²+ûuF?ÃöÔ{J·?Àý²+ûuF?í¦kd'ù?º\ï€g)Á?²Ì¤Ü¡^¾?º\ï€g)Á?ìsñ{¥4O?«8ÇjóŸ?¼`t"Ö]‰?«8ÇjóŸ?èf«Ìˆ??°3Ióè?ÎePÍß¿?°3IóèAGN4FGL J1829.2-5813¿èå	trîŠÀ4j½ãû½À8†‰À;–lÅ%8Ÿ@­ŽE'§d@rÑ®³Ý?œ€4»Í?ÀXƒ#á\@`^åh¥@
t÷"ᬿÑAwcä«ç¿ãÆ°žBö ¿èS]õÿv¿æë+Ý~uÒ¿ìIìqþ¿ïÿî' ÇAGNfsrqPKS 1824-582?ïÑ
s[?­ŽA·/£?wzƑ¿›?­ŽA·/£?ïêû²#P?s"~¹Õî?eMèü8a?s"~¹Õî?ïN€&^—?"')Ám¾·?–/û2uO?"')Ám¾·?ïÿBçlq?°ŽßÈÈ?£§M	˜?°ŽßÈÈ?ïۍ©\–?sDöOC?r{¹ÔÔñ?sDöOC?ï—£ˆl?¡ŒËÔúú¥?Š=$Ä6z?¡ŒËÔúú¥?ïm»w?'	+ÒàšÜ?'^}¬¹?'	+ÒàšÜ?ïü%j{R?7G¦n??†ÕŠ?e'?7G¦nAGN4FGL J1829.3+5402?؏üöôØ@8Ìñ`®—À9úVÔ"+¤À<d?³t63@ 5q4ˎ´?û©Ø@žUÁ?·*KØñsJ?½Á"o:öK@õM¾Ñb@9{E¼D¿ïå!4y?ï'~ nö¿×—ñ"íjÒ¿Ö9ñ'õèO¿Þ‹}ÂM—ã¿â'«@‹AGNbll3FGL J1829.4+5402RX J1829.3+5403?ïþìf
:?<õçÌ"?!?§ûXñ|?<õçÌ"?ïëâ.çQ¼?h©W<R?dÐÞôÔh?h©W<R?ïô²/?Iîî2F…?V›Ùø÷ӂ?Iîî2F…?ïÑxÏäH-?Ztqp?wC˜ú1>?Ztqp?ïýËíÔ¯D?+:‹Ä6êI?1 '5#·H?+:‹Ä6êI?殺­ÿ¤ˆ?šdj<þ›Î?†"Ôy7¦?šdj<þ›Î?ïîLQšÚë?kÆæšÝs/?a³®[†-=?kÆæšÝs/?ïb ú=?'¶eNX¾‹?"»àªõîv?'¶eNX¾‹AGN4FGL J1829.9+3934?ÍI"5"F@4ȕá~4¹À:Ðw/†FÀ<šã'áït@HK×Cô!@"ýØ?ĺ{B?·ÉÓH<ç?ôÿ5ºÌð@ê;ò•í?ð¿ä:'
‹þ¿å—Î=e;C¿Ù¦DÉ]­¿ë&i@‹`q¿ïånN'4KAGNbcuNVSS J183003+393638?ïîÔÂö›d?ZL|ÖÐfÌ?a+=&ATS?ZL|ÖÐfÌ?ïÓ4×v,?wæJ¶ØOÕ?ve"š±e¡?wæJ¶ØOÕ?ïºUÓ¿ì?{VѳêeS?j¾LÇÒê?{VѳêeS?ï\OÊv8õ?sG«ˆ÷?"vªY©k?sG«ˆ÷?ïÙ»B`Í ?q>%¬™Dð?s"^ç¦sÆ?q>%¬™Dð?ï+F×ð?¤ Ǖ"@2?š—=‹á&?¤ Ǖ"@2?﫲~lí?ˆ/á1BI$?…9ÓgCüœ?ˆ/á1BI$?ìý	Ú/
?œ—/ÉUÑ?¸±,ËIœ?œ—/ÉUÑAGN4FGL J1830.0-5225¿ïS"ӝ\®À2ÁLf
À:É20Ô´"À<lý@´%@5ՈJø?ùÞ Ô÷=º?Ö%>}êª?â¯'9*Ä@Ü;\Í`q@@DˆE?íº¬Ùè>B¿ïÏÖÍ׏?î´ýØÞS¿×'Ï<h¼¿ìCÌÞj"¿ïüDôü–¿AGNbllSUMSS J183004-522618?ïø$|61j?Rd¤=6?K?On/yfˆ?Rd¤=6?K?ïåNLØåy?tëà*N?j±³\´o?tëà*N?ïÐà‹N0?AºÈXíÚ?¥ãó½£û?AºÈXíÚ?ïr®À"¨?vçž‹ªÖ?ˆ£TLk:!?vçž‹ªÖ?ïê!ºöò¡?pmæb–i?eÞE$Š>?pmæb–i?ïÆpŒÚïO?ƒ(oªn¾N?|ǹ™gJ?ƒ(oªn¾N?îwªyáJ?Ÿô>WˆåÞ?¨…Xp¹¹e?Ÿô>WˆåÞ?ï`ªV͎‹?š½=à Â?"êµ(ü›?š½=à ÂAGN4FGL J1830.0+1324?ÈóÕi˜9@%~`ÔV.À9é©óƒð»À<	‰±Å	Š@Ä{MSDö@SZðç^?ÀHjýÏÏ?±–c?{§'?ôúkÖ证@	€ãäky÷¿Ø´ªagùä¿ê–à·e\{¿à'mb*W¿à,&Ïw¢¿Ý:¤OÜ¿è‰52ç³ÙAGNbll3FGL J1829.8+1328MG1 J183001+1323?ïýˆc¾I?$ã"K/?3»ƒÜT?$ã"K/?ïÄû¼X>?3	d$9=?}'u©cï?3	d$9=?ïóè'{M?XƒPOÎGj?X.ÛFJ"¹?XƒPOÎGj?ïõù` öý?:=ïºc™Ó?T
?#Æt"?:=ïºc™Ó?ïú>¼ö]?=Ž"jR?GéÍË?=Ž"jR?îdÍá$=?´ª·y–~c?©³!îÑÕ+?´ª·y–~c?ïæ9÷-ڕ?u›Æ¼/Ð6?iÆ	_zÅ?u›Æ¼/Ð6?ïÜOývìN?]^hÝ6kë?qØ[ç0Í?]^hÝ6këAGN4FGL J1830.1+0617?'OÙ£G1á@Wáá1àÀ9<•ÃKCËÀ;‹PMö-@qV…sÈ@Ž£yè#?¸´¸ƒê…Å?·ÎFO?ü#ûØSÍ@z$n?ïÒjeÏg²¿Útî¿eÛý¿äÎ×ؙŠ¿âHŠèü®<¿êÒûºöás¿ÜÉÇÿÞrAGNfsrq3FGL J1830.1+0617TXS 1827+062?ïú8Ä}Ú??©÷÷ÊR?Gî;¸{j??©÷÷ÊR?ïʕ€bïl?Ž"A{º?zµ?Úæáæ?Ž"A{º?ïÁ Äe?|.ÞoÎxU?/ýž$i?|.ÞoÎxU?ïþZð«=?=8!Å|?*Pó<jú?=8!Å|?ïæQP³)k?g…<œëÂ?i®¯+ÚTò?g…<œëÂ?îãÉ5
?·º}l~?®Ãj÷]?·º}l~?ï>' 3ì?'Ã`[׺?˜;~ºw?'Ã`[׺?ïýÒhSb?.q0:µ6(?7ÉkÕe¹è?.q0:µ6(AGN4FGL J1830.2-4443¿É¢¯,}âYÀ.jÞe{"ÜÀ9BW@X¶À;é·B÷ÌU@'²^Ø(@L~ä­³?³XÚ©¯;?ͨœkÛñ-@Ú:_w^Ü@íÇBŸ6ç¿É6$ª.gG¿àG¯â0aG¿è¥ú?÷'Ç¿èeÞfRD¿í`b@fø¿ðAGNbcu3FGL J1830.0-4439PMN J1830-4441?ï¤æÉùé?‡tâfMM!?†ÆMsÿ•È?‡tâfMM!?ïë׳Ÿn	?z;|†¤üz?d(L(8_˜?z;|†¤üz?ïw2ç]ó?'^ɹòÕu?ŸQ£A«?'^ɹòÕu?ïþݜŽý›?ÛÌG|èL?"&7€LÊ4?ÛÌG|èL?ïØn¿âiÓ?yN:vòó?sÈ êR?yN:vòó?ï™&ë™?¢é;Aš`0?‰¶{ˆ©µ°?¢é;Aš`0?ííˆBˆ´? N(ÁÉ?°"½ïÉ­Ý? N(ÁÉ?ïû?ì œz?7q'6Y%?CNÏÕÌ?7q'6Y%AGN4FGL J1830.7-2713?ïúÂå~…¨À"jP
_À9—ìoîÀ;¨uÕo3@nƒGr°@b¢§_U?º¶ñ™4ïÌ?¼Ö€TÏG@<h€òÙ§@u•ßû¨­?ïŋZ;µ¹¿áýwå?¿áýÖ?<Uò¿ÞÊÒ É¤#¿åÈ¿nÀR¿ïþ؃ªDAGNbcu3FGL J1831.0-2714PMN J1831-2714?ﺆØ2å?"šMSö?^IòÊZÕ?"šMSö?î›8ä‰=<?ªA)]ׄ?¦Lq¹#ú;?ªA)]ׄ?ï—ÎEü?"æÑa	P?œ¼,ÿX?"æÑa	P?íËÑ!è?'ô_-¥I?±ã§È->?'ô_-¥I?îPzn±?¬©"ëÀÂx?ªþX9'?¬©"ëÀÂx?ç1ƒ¸±·É?ΡÄ"%¼?ќøŽœo?ΡÄ"%¼?í–8æüN?©¥õ¼g÷L?·#N8È'?©¥õ¼g÷L?åØÙö£W?±gä*a}s?ÔOøL¹Q?±gä*a}sAGN4FGL J1831.9+3820¿è¨éj‰®@4š€If{À;Pz9'ÍÀ<¾Ýšzj)@ cnv*S¼?þ†Ôš÷g«?ÐFðù²?Ð2?"?ý,©@։å@'ԱÿîÂë'D"X¿ëöòoô"¢?ïþž¦ž»¿àԄ¡ºÐK¿è"PïܜN?˜bãz
b>AGNbll1RXS J183202.2+382132?ïözµþª?PH:OTÒ?S
"ý,væ?PH:OTÒ?ïå']g?o'`·ã?já؏[!Ä?o'`·ã?ïÄÂáØ?|=2o?}žósã?|=2o?ï®Ð¾Û×?pÁš†×ß ?"KÐL®æO?pÁš†×ß ?ïÖlÄU?q:Ÿ˜%)?töI˜±Y'?q:Ÿ˜%)?ïq 'Z…Ý?™ÍЈS?'ËíÒ÷vS?™ÍЈS?ï½·ƒÃ?"E?º| ?H\*ÇUŸ?"E?º| ?îásYá?B?'jPé˜Â?¡èÊ`4=â?'jPé˜ÂAGN4FGL J1832.6-5658?à"]âM+qÀ4m?ž{À9d8F˜jÅÀ<"a+"@qƒ¯½@"+¶g/º?±œÅžbe?®±±à¯¥?ú*M`Ûâê@ÙFœF?ì.¾¯R¾¿åt…
›¿à4º-ô¿àP"AÉN¿å<YjÕa¿ähÁTɅðAGNbll3FGL J1832.4-5659PMN J1832-5659?ïý—ߊè?#[ÏzB†Æ?3A"^¤?#[ÏzB†Æ?ïòü‡Ù?_/P3vài?[þ —‰?_/P3vài?ïö)¸"¸b?XâyMD¡?S¬ŽîŒ¼o?XâyMD¡?ïà}ØGï?Z½¿Ú=H?o''нÿ?Z½¿Ú=H?ïùôÔƒÖ?AKừl?H,¯²öçò?AKừl?ïÒ6ژÎ?{'ÖM&hè?v䒡
ܽ?{'ÖM&hè?ïî$ÌÏ7F?o«~PlnÞ?aÛ3M¥q^?o«~PlnÞ?ïœ3<mn˜?xëÈ»?ˆó0ä¤Yç?xëÈ»AGN4FGL J1833.6-2103?íyÔñUæÀѹ_1¾¿À6`°Å/JÀ:‰"ªNô@¸£Äë¬â@¦v§&J?‹­IòèÔ?¸eúéHÙ@&¬`gHäu@Aóâee¿Êg>ÀZ#¿ãÀVgâ¿çlë¯#¿ç%¼R+F¿ê>ùºì¿îö÷ãÑÌAGNFSRQ3FGL J1833.6-2103PKS 1830-211?ï€YÆ^¸?Ž
¤ÿ]¬?~¿Ó#7ï?Ž
¤ÿ]¬?ì¤Úüvš?Äõ‰j³Ž?¿2Ù(K2?Äõ‰j³Ž?íaFîô6k?¦àºYF‡?´õȉ¨')?¦àºYF‡?ï©-îJ0?}üaí]Iˆ?…´"u}Ø?}üaí]Iˆ?ïËMê!O?uPD¨[íQ?zY
üfý?uPD¨[íQ?âÀ,±Êùõ?Ó!¤'*›p?Ú¦œj?Ó!¤'*›p?îÒ剌©?™D>
ûÂä?¢Ñ®èCv?™D>
ûÂä?ëlÌ	a\?´'éŕ›¿?ÂLÏÚ{ê?´'éŕ›¿AGN4FGL J1834.2+3136¿ìOp2ÂõÞ@13¬)ÜrÀ:˜T+
pÀ<MAî·Ù @!6âågù9?þEäæŸê?ÌüŒ¥ä?²{;4´g¦?çu *­R´@ç™ZÚl?ïêõ6¿åŽü¢}mê¿ì›'û? \¸<ÇÜx¿ÝmmVD°3¿åÛBöAGNfsrq4C +31.51?ïùì.€µ·?E䵏MAs?HOEՔt?E䵏MAs?ïãìfΞ½?p¨«g›q?l™sYÃ?p¨«g›q?ïÞ)Î?u{-Õq¨6?pëwœšÑ?u{-Õq¨6?ïÙ~Ì
?V‰w¯ÜH?s@·£˜g•?V‰w¯ÜH?ï迨]=?e𣤳ö·?g@W`Ê}5?e𣤳ö·?ï…uomÌ?•"¯šqaÀ?Ž½â§"(ø?•"¯šqaÀ?ïѕZ¤f?}d片?ß?w5r: ˆù?}d片?ß?ïLÙµ=?ƒ—̕å?–dÉTރÍ?ƒ—̕åAGN4FGL J1834.7-5858¿ï‹¹wŽ	¡À4ñoiÀ:›ËáªÀ<6h¯ìÂ6@¬Bè2@'V¡ÍDÂ?Ð6Ö@hûÂ?И
M`Ûã?þV>J¾j3@	(#á≿ï_jÿR[?ïãyòÄ-¿åF;Šsâ¿ä&vVžrF¿îÚ"ö¥
¿ïþs£eË6AGNbllPKS 1830-589?ïóß3µ?SdÍkÏx ?XAÿþJAÆ?SdÍkÏx ?ïïRáNd?bu¡ë>QE?`­ÂÈ?bu¡ë>QE?ïyŠAÚ7f?"µì`d?Î·Éà}<?"µì`d?ïè¯|wÖ?Rü~Êm?gPƒ±ÀùÐ?Rü~Êm?ïëÊ&\é™?d1·i*"h?d5ÙÐq?.?d1·i*"h?ïÈP笪¡?€^« o>?{׌G7ST?€^« o>?î¾eÔ£¹a?™K÷äÎWY?¤¢²TÍù?™K÷äÎWY?›¦˜?'Y>D:?ã?–,Wéú?'Y>D:?ãAGN4FGL J1835.5+1349?í>X>ãô@#pxú½ àÀ:^qhøçÞÀ<´-™–?@xD6¿@M|Š•?ʪ < ð%?Ç­NWPôº?ÿw¶4ÚÓ @ðÓQÌ%ˆ¿ïÞf"‹=?ï˜j$aY¿ãB#%žõú¿ØÏ= ˜ò¿å/¼»Ý'@¿ïúDŸlArAGNbll3FGL J1835.4+1349TXS 1833+137?ïÞ²ÓÚæŸ?ªéE°6´µ?p¦–'*X?ªéE°6´µ?ïXÿP?ž|pw66?©øwА	?ž|pw66?ïφm—Þ?woA_éÙ?x<É"Ñ?woA_éÙ?ïÅZZna?anŸ®Âá?}R±W˜C¶?anŸ®Âá?ï馊ñc?m,¬cÿ6Š?fYvH¬]?m,¬cÿ6Š?í1Fýü€Ö?»'ˆ\&ê?¶uÈd+U?»'ˆ\&ê?ï!Núíz?•å_
Ðæ?›Ö ¤Š?•å_
Ðæ?îꈟÿÂÌ?'HKL`?¡WvÓA?'HKL`AGN4FGL J1836.4+3137¿èéWYë@0ÇQzF<À9ÃÈXÉűÀ;ã'‰±Å@·5ôƒ @ð%ï?¶‡Ü¾îy?žsÚÔ?å£|f'ì@	'tΉ‰?äPŽù,§(¿Ýùà4ì¿á)½h«»¿èŒö%‹«¿ã{6l£—I¿ÒS<}‰ÃŽAGNbll3FGL J1836.3+3137RX J1836.2+3136?ïü€Ç:¼"?28'ÉÀÛ¬?;ùÅ/k?28'ÉÀÛ¬?ïêú%å0¶?qŠÌA?eÚ>‹:5?qŠÌA?ïÛ«t¸c´?xèýîw~Q?r*E°Ü©Ö?xèýîw~Q?ïìç~¡=?Iæ¨9ÓÓ?cŸ[‰@?Iæ¨9ÓÓ?ïçÖÚSn?d¾ÓÜC)?h)%·ûQ–?d¾ÓÜC)?ïšþ|®b?"qæHàÖ?‰@`ÛF"?"qæHàÖ?ïµIÃE?…£ôú-ý?'­,qº»?…£ôú-ý?ïµ	{m£`?l½'k¥v?'½¡ éÿ?l½'k¥vAGN4FGL J1836.5+1948?Þ$9¶3k@("'Ù±·žÀ:#GÃEeÀ<(¢¹ÓËÅ@tˆ$QC@ÖïÞIÌÓ?¼M3y…'?âmY09?ÓÌô9ù ?úJC*L.Ø¿ážf½¤:Ý¿æDw(U‰Ÿ¿ã F&Tþ_¿àËx¤V‹þ¿Þ╠Ž¿ã'¸ú‡ñAGNbcuNVSS J183632+195047?ïñë3ƒÿÃ?UGÇëjµi?\)˜Šú3?UGÇëjµi?ïȒR±?‰Ãø›eTK?}¹¶¿úc?‰Ãø›eTK?ï܌Ññ5?sÌÈðõ (?q¹—Ä	Z?sÌÈðõ (?ïÁé´0–?ežöË\¸?%î",N?ežöË\¸?ïÈëMÃ?ucÌËM°]?{þŠ—ÅšY?ucÌËM°]?îíàúguì?¨¼¤u:¡?¡!ðX¬º??¨¼¤u:¡?ï²[˜N?…4s¢ë?ƒyitÞ³?…4s¢ë?î¤@\oP?'õ³P?¥»ú9
ý?'õ³PAGN4FGL J1837.0+5347?×bL£7b@7£¾ýq?À:"
xÀ<nCe°^@n]ST0@Ê:KUhè?µ'éÀè+迅Ln:Á?Í+éþ5ûe@æ åhã¿ÔŸ¯=æÜ¿èT×È©Qž¿çõšÀ[¥¿ãXˆAØg‹¿ë>"_¦XÅ¿ïÿ˒:)ÇAGNbcuNVSS J183710+534704?ïòÈÂQÕ?Rœåu-ˆ2?Zn{&»?Rœåu-ˆ2?ïôrÔ;‰¢?X\ðyÚÌg?WW_±m*?X\ðyÚÌg?ïÅöPB§^?¨2ó¢•?}×ðŠHÆ?¨2ó¢•?ïãÚÁ	Ӝ?WÅ=ä»L?l%?
Êç?WÅ=ä»L?ï̶°y?sú‡ëÓ?†?y¤§öó̟?sú‡ëÓ?†?ïËúKØh?z"aÐßÁ?zÚ<ڕ?z"aÐßÁ?ï\lg‡N?‹o/™½Ú*?ˆ¨äðmƒ?‹o/™½Ú*?ïz}³ù°õ?€zPû†xÉ?°I'¯U?€zPû†xÉAGN4FGL J1837.3+1052¿ï-ÆH	•@ '5ø	'À9ÙúàŽµÀ;±Àn¹@gýY‡…Æ@b<ççÛ?ÕvŸC§ ?ÃQ]?ÌÐ?ÿºC'œüû@9C!ór?š¾\È¿Ýà鄓x¿ê/·éùr¿âu>`bì3¿çôñ^|¿ïÿûÎBÓAGNbcuNVSS J183713+105143?ï÷ƒnÆ?Rcè¨bš?Qþù'ó0Þ?Rcè¨bš?ï¦EYjC?"ÁÖ¾ý§?†x.¦5Ó.?"ÁÖ¾ý§?ïŸ3ªì?ƒî»÷÷Ï®?ˆ>ÿ(Æq	?ƒî»÷÷Ï®?ïÛr*?RäeÛR&ã?rzqÑú—4?RäeÛR&ã?ïL¤‹¦/?™d`Äê>ó?–kn ã$?™d`Äê>ó?텋±¾B_?¼·ØÛ	6Ç?³Ó¢sÅ»?¼·ØÛ	6Ç?ìê<ZŠvL?ªª¿™Co?¸®*bs ?ªª¿™Co?ï8æ×B¥?m»cP®Ú?˜ã%ø$?m»cP®ÚAGN4FGL J1837.4-1646¿è…g0ÂÀ9åâGˆUÀ9šsfÿéZÀ;úý9@.Û'X‰"@¾+Uï ?ÕOƒ3є?åAˆËëü=@R
Á‰¢¬@å?ïÞþ"v¿ÓtnÒE²'¿è<Ÿ9@>¿î¾£%¿ïÿÿ)@k*?ïøš°ðÎ4AGNbcu2MASS J18373301-1647530?í¿-k¸?Àöæ?©R?·7:Lp??Àöæ?©R?ì]ßeš}^?ÁPæ=rb"?½Ó,?ÁPæ=rb"?é"3AÝ]?®P4ü°?Ëw2ø‹þ?®P4ü°?ì¼×6]49?¡B0Émê?ºFM^;?¡B0Émê?èòx¢?ÈÃÁ+?Ì7Þ§Ýw?ÈÃÁ+?ÕŠˆôI­?ÐÉn̙ÿ¤?åpº»…Û)?ÐÉn̙ÿ¤?áçD²·wÑ?µ˜?¡Êx[?Ü1vš'^?µ˜?¡Êx[?ßb'Šþî?¿˜…Ðívn?àNô¶º€‰?¿˜…ÐívnMIXED4FGL J1838.0-5959¿çîiÞ§&À5¦¾zúr"À:®Èú°4çÀ<~PŽÌÝ@ ÀR¬u>p?ùÒk<Žüˆ?Ψ£!ؗÜ?Òw¬tg°é@ò¿-§Ù@¦žûn¿è›¤¡4˜Ž?î(ø|}ÿà?è7é{Y=¿ÖXF½ÿ}¿á\LœÄß¿åPŒ?>qAGNbll3FGL J1838.5-6006SUMSS J183806-600033?ïüqk/×g?3ÆÈ
w&?<t¥áÖë#?3ÆÈ
w&?ïâ3»?öð>ÆT-?mâÍ$Ã|??öð>ÆT-?ïÏÿ·ä;?vÈâ|?x€2|>i?vÈâ|?ï¸76x+?iEÓ‰ûµ?ò2c×2?iEÓ‰ûµ?ïù¼'ãÛÃ?F ŒqøŸ?I
ó›ÏŠv?F ŒqøŸ?ï¨Ìõ¼…,?–¸IØÈí?…̐޵?–¸IØÈí?ï¹}GmA?…?¡Ý^5-?¿ ³¤Ê?…?¡Ý^5-?ïJî×Zh?‡‰åðªå?–¢%"\ø?‡‰åðªåAGN4FGL J1838.4-6023¿Ûk]œoÄÀ5Î/ßÁœÀ;Â~•1UÀ<™7¨ùä@!aéÆ,ʎ?ý¹Y_ç?ǐÈû"?–†¾(LØÔ?Ñcº¥@·ä$\V?ïå$|·
Ä¿ä¤ßßÏ^¿åOV_2?˜¿ÖE@[º»Ó¿æêNˆ#O¿·ø'wAGNbll2MASS J18382063-6025224?ïÿ…TÏKh?hÎ7>ã?ªÏ¨'?hÎ7>ã?ïõÉl½e?XU	m.?UÐm.ÄF?XU	m.?ïùÍî­>´?;JnŸ®#D?HÈENÞWô?;JnŸ®#D?ïýÐÈ:l?›:éa+'?1›Ê¤1N?›:éa+'?ïÿ®Žž=î>üÛ=V,"¤?\["¥ºÜ>üÛ=V,"¤?ïÚOhZº?€ÒÃ8{Õå?rØL
O"?€ÒÃ8{Õå?ïù«#ýÀ?bNf	0?¸?ISpå­
›?bNf	0?¸?ïùÃ-ÚC?:rfx'³?HóL]«
*?:rfx'³AGN4FGL J1838.8+4802?"|My°í@5҉üm¤HÀ8Y…O_¹¤À;'*è´@¿õ=Ú+/?ü9"ù÷¨?¡Dª©â< ?§Í?¹Ss@¢ÁE°
y@#3d1¿ÓbÛ, Å¿Õà¢A³Õ¿à-n}ŒÙ¿ÔhrÛâ`¿à¡u0.¿ÚÍÒ»ú²AGNbll3FGL J1838.8+4802GB6 J1838+4802?ïþˆÔzk+?sñ ›K?'r»Öü˜?sñ ›K?ïò,ãìV³?`³ÒÂ:µ?[¦7®`YÁ?`³ÒÂ:µ?ïï´ÃÁ‹P?_gÄ­c?`K<»@%?_gÄ­c?ïÿ"fv}?	ãuõºTv?³8oxfˆ?	ãuõºTv?ïýÏj9®?-0h—'³ü?1"°¢S=#?-0h—'³ü?ユ6³pZ?Šq(K€?€Z²JŒãu?Šq(K€?ïëí–hY'?nñQ77a?diªä¨µ?nñQ77a?ïþñ6's%?ënãbý€? ì™kx£"?ënãbý€AGN4FGL J1838.9-3457¿Ñ¬®·qÀ)—¬>·Ë´À:NÒàD²À<DÀ:î˜@#ݤ
‹Ê@®È b?Ä	çƒÝ?ßa¯²à'|@Ž6Kìg@ðÜvü?ïø©"¹`?»-(­Z¿áÌHþv"¿çà,€f—º¿ï¦tÞÏ-пï­ðÔ+AGNbcuAT20G J183923-345348?è˺à›?Ó¨÷sÍ?ÌѼ͖?Ó¨÷sÍ?èY!mÒ°*?ÅZÈY(C?ΛzHµ?V?ÅZÈY(C?ã™~ru?³>è 6í'?ØÍ÷Å?³>è 6í'?ë‹éɀ›?înËRÐ?ÁÐ[àÙý•?înËRÐ?Θgëó"?Í5Ùfõ=À?èYæ ?Í5Ùfõ=À?Íy¯×§#ù?Çn&	2Ï?衔
7?Çn&	2Ï?ʓàXV™?²ŽÓç_i?é[éê{?²ŽÓç_i?ÖôRڏÐd?±¡{aáw?ä…Ö'¸Î?±¡{aáwMIXED4FGL J1839.6-7107¿ïŽ¾Oœ.À8ŸØ­«ŸVÀ:ƒñ'¨4À<l'ÐR@&ò	GQx@a<á1ޟ?Â6‡»öÁ?Ño^|âÿ"@ƒ)›üå@J肊ßB?Ð%óD/Ú¹¿æ*#ŸÂR ¿ê܍YýL¿ì\e'TPº¿ð?ïÿÖ°cAGNfsrqPKS 1831-711?ïæÑûWF/?u0é‰t1?i.ãÓR?u0é‰t1?ïôþ+{õ?YÀ–RNA?VªnzõP?YÀ–RNA?ïZB&ý+?"d[ô³Ì?ž"·¹hŒž?"d[ô³Ì?ïý™%€m#?#4¸ªê?36ÓCß?#4¸ªê?ïêá
);ì?s8,fH;?eóüã‹?s8,fH;?ïÔ5ØÅJ?(ᆇ·?uåó®_8?(ᆇ·?îtŒéKÍM?Wbø?¨·1i‹]6?Wbø?ïèÈE.?]š?5dÛ¶?g7èÅ=ñ¯?]š?5dÛ¶AGN4FGL J1840.6-5545?êÌÙYøïÀÀ4²ôàM/À:"µÄr‹8À<95>»@N©•·b@i¦Âwu?ÌF³Ã'dÂ?Îå=F‡xÛ?þ{ƒ@GþЪýÅ¿¡1=ßoοÚ]7þôè¿êßß~€8 ¿à‰T!ÀD(¿ïþ_–}Û?ïÓä^
ýDAGNbcuPMN J1841-5544?ïöýìeª?Psä‡3O‹?R'¨¿{?Psä‡3O‹?ïóëEøvŽ?_#Á«§}?X)tr¤M?_#Á«§}?ï:Öô ¬?ƒonƒÞtÕ?Œ±JT%àÔ?ƒonƒÞtÕ?ïÿ֏nG†>èEÙ?':>ô¸Rï@‹ß>èEÙ?':?ïü d…r?<÷hJÛ«?:üáÊN}=?<÷hJÛ«?ï×ï	+'?ƒœóÕË=?tws+'??ƒœóÕË=?îâ‡ôxê?—BŸ"IÊÝ?¡×€µ%d?—BŸ"IÊÝ?ïÿ7ã=žé?saÊð<?"'\eÞ?saÊð<AGN4FGL J1841.0+6115¿ï¾¯¸"Ü@8ÉzÝð,À:+ª¨µ–À<"˜8p‰Ö@­Z—@iøÂ!?¶e Ÿa¿"HóÜ'«?Üùm'e™@šš?íˆZ吿çs×¾}J¿ë%§>Ê¿Òft©H›¿ê|•aütZ¿é‰@»±òVAGNbcu3FGL J1840.5+611687GB 184000.4+611120?ïû1ȋ/Û?@g`¦h5j?C8Þ·f¤F?@g`¦h5j?ïö±RF?Vä³­âÝ?R[Þ¶£Ò?Vä³­âÝ?ïß*xࢩ?p©{ÎO'?pjÀc±?p©{ÎO'?ïüá5A™?#ÕEh8'?8öXÒß±ù?#ÕEh8'?ïòÙk2?SȦ5×ýÖ?ZMÞ$œc?SȦ5×ýÖ?ï×P̅ï?u'gB¦»
?tWù‰îÔ¨?u'gB¦»
?ïÉ"xh¹?iSX%0À?{nÃüw?iSX%0À?ïö—Äà;?D€ýú6¤?RÐv¡YBó?D€ýú6¤AGN4FGL J1841.3+2909¿Óg°Òµù@-±«ŸU›=À:Vî#^ªÀ<)Æ°Sƒ@!ÏYè~¯?ùP¬:†
Ì?Äd?D¹mt?ÃÄ©Ü¡V@nÊhn~c@ØíÙ6èt?îæ{_ïJ¿è±Š¼‡l¿Õ"!'—ô~¿Ó«é]&KÄ¿ÁƒZèÙÉ¿ãúM~caAGNbll3FGL J1841.2+2910MG3 J184126+2910?ïäñ|k?sÄ}¸·Ï?kçöü¥S?sÄ}¸·Ï?ï¼Î-†1C?‹¸¼œun?€ÌtŽýqK?‹¸¼œun?﻽nF@?»šª££?<Pšœ?»šª££?ï@G¡\å?pÞƊká?‹ïîb·?pÞƊká?ïÎTž?žcmÆ1?&5…EÁ?žcmÆ1?îÁí±Úê?±h+ü´Ñ@?§á$j^?±h+ü´Ñ@?î52Ûä0°?¥ìF*Tê?¬¬ÒA¼ôú?¥ìF*Tê?îîƒ<J?b¿G;~?®áËbdZ?b¿G;~AGN4FGL J1841.8+3218?ËwÑþdõM@/ô(²¦°ÙÀ:&jö±À<'-Z¬@ h–=º6?øå'Á(?È-Š½2Ðã?ϓºÝa @ËýÝï@
¹é¹S?ï×O!¦Bõ¿ ´T0ý¿â4»ÉoJ;¿£\|$56¿ÙÕÁ½ú÷Ø¿êÒ]«AGNbll3FGL J1841.7+3218RX J1841.7+3218?ïöKóbQž?MovÒ«³?Sh£Ðä8?MovÒ«³?ïÖòL…Œ?ƒá"v;*?t†Ù®® ?ƒá"v;*?ï°&ŽÚ?'iròÕ7?ƒþ¶W¬?'iròÕ7?ïì§È}Õ?KéÚ(*?cX7^oÔ?KéÚ(*?ïêY¨ÆeÞ?i4\쨪?e¦W.›b?i4\쨪?ïJ!ÀÞƹ?¥
©Û"áŠ?–»Çä'(Û?¥
©Û"áŠ?îç­¢m0?–®@?¡….ú$¯ô?–®@?ïÆ](ò^ú?oÄÜ=ƒN?|ÑkiCß(?oÄÜ=ƒNAGN4FGL J1842.3+6810¿Ú&É "'Û@9à(=5ëtÀ:5óÚó×À<FõÉEXÐ@"ø4.°Ã@.d"Õ?¾§à?†d?³?ÐÿŒh?ñ{½•ø$i@ëóbål?å}>" 
Q¿à²ù¢í]¿çýªðÙòO¿çV²X­@¿åÿ~?ËòÝ¿ïý:ˆ'
YAGNfsrq3FGL J1842.8+6810S4 1842+68?ïþ`²L?"³/Xl4Z?/ÉôÓøR#?"³/Xl4Z?ïô]ld#¸?ZU}Œÿ÷?WE'qqþé?ZU}Œÿ÷?ïï0žr5@?kºZ)žÁ?`Ïa–	χ?kºZ)žÁ?ïæ.@7Ü?P3ȉ8$?iÑ¿šÉH?P3ȉ8$?ïý¹<Äy?2eAܽ'°?7b7¸`IÞ?2eAܽ'°?į̈СÌ!?Òl`Øs?y«—À÷çŽ?Òl`Øs?ïæ%;"ë½?pêR…½%†?iÚÄêÒ²š?pêR…½%†?ï']¢iï)?vn?¯]4?h—hóÑ¢?vn?¯]4AGN4FGL J1842.4-5840¿æY—$c%ƒÀ5Í!…Æ~À:'FÙÙ$ÊÀ<kÕW2@!ßX6øº'?ùµ>U¦$Â?À¹e¼ÈGØ?³ÒÈ ~vd?õÂäßJ@c?cÃ÷¿ïv³…Óé÷?î϶¡'6y?¥'@"ɝ\¿Òëý?Ò¿à±6¤û©¿ÇNògHºAGNbll3FGL J1842.3-58411RXS J184230.6-584202?ïÿ,|Ïx=?6q´b!è?pm)]‹?6q´b!è?ïõ9õ¼|•?WžAÁºÎ´?UŒEVu?WžAÁºÎ´?ïõÿæL0?T®J:ì§?T3ˆÃàv?T®J:ì§?ïþ ˆºèã?fRò"tÄ?%÷wæoêD?fRò"tÄ?ïÿV¯0§	?(·–j?*"mzß?(·–j?ïÖhrìAî?€"q ?tËÆh2Ý?€"q ?ï÷®@€ßË?VæZQ('?P£qº)?VæZQ('?ïýô'P¹›?'õ%@·AT?0[vXM?'õ%@·ATAGN4FGL J1842.4+7613?éŠ*M'ó[@:ўùTëÀ:þ•{&çËÀ<zŒç¯¸@ߖK±YT@õ"yŸ(O?ųoC.ÓÓ¿±pþöÌ%?ꖝ^Ë@ÐÕ¹ÛX?âTO­¿ç`|wIãy¿èHèÜÍËпæ¸þ˜¡Í¿ÖÎ9Ì¿ïúµ¾=gêAGNbcuNVSS J184225+761046?ïþ†"^?0%(°Sì?/瞝~f?0%(°Sì?ïôâÀ¤?YóüÁÍ?V:~Ø­hŸ?YóüÁÍ?ïÝ&¨Çp?{Áuÿ×(U?qsl¹Z·Ù?{Áuÿ×(U?ïûÂۜ7?-[óî:4ù?@ö½Š"¥?-[óî:4ù?ïþ—äÒkâ?0ËrY"èí?&±Ü^¢¼?0ËrY"èí?ï˹—Ä_ô?x¾"j"v?z#4
Qåä?x¾"j"v?ïà[b&eÅ?y|Â4v¶â?o¤ÃœºÈ?y|Â4v¶â?ïÒ{ÔÑlÞ?mLÏj¤¢+?v›iÆ?mLÏj¤¢+AGN4FGL J1843.4-4835¿®ÜdÍ¢KÀ2Ág#$È6À;#jJ µ'À<"Þ·°ÛÕ@ /(Œ't?ÿŠ"¢Óä?ÌGOŸÐjf?²ÐË_ƒQ?꤫`kz¢?ù!¥AB•?î"þ×áÓÅ?ï™G™ò"í¿Ô'd=AT¿éÈ»ÆKç?ÊSk¢ep¿ðAGNrdgPKS 1839-48?ïý¦Õ	c?9¸,@ü?2ÉX6"¿?9¸,@ü?ïÜD•lt"?ƒÄ³ÿèØ?qݵ`s*?ƒÄ³ÿèØ?ï¼»˜¾?€ó=s®Æx?€Ñ?A™0s?€ó=s®Æx?ïð'óžY?NË%×)Â?^Ú]™Œ!?NË%×)Â?ïýÙÝ*Ç?:µ‡õÇ)?17púr`?:µ‡õÇ)?ït•R&`?§1"¢¯å?'mUÀg=ñ?§1"¢¯å?yÀ,Î?†fɅÎ?‡Xᅥø¡?†fɅÎ?ï§úö´Zn?øë§?†BOyȕ?øë§AGN4FGL J1843.8-2011?¿:Ë`™¦ÀЃn—À:§\ŠD'À<\W=Ôvå@Þ^eþj@Ðg¤T?ÎÁ#vQÁ?â":Re@ÚÙºñØö@ÑË«`?ïÿ΁ز´¿È=䧉ò2¿´l¶!9¶…¿á[ā¤°N¿îɟ†B¤À¿ïôÒÛÇ5AGNbcuNVSS J184339-200606?䃕7yã?Ëg?»h?ÖøՑ
ü9?Ëg?»h?ç‹o_fö?È3øށ2Î?ÐéÃ!A2?È3øށ2Î?èWxÓ·ˆÔ?±¹á™)?΢±!Ü°?±¹á™)?è¾hZ?¨a H£F'?Í¢^—É?¨a H£F'?Ù¹<õÝDó?ËÝ$£Ä?ã#a…]‡?ËÝ$£Ä?ÒsªÃHк?ÏmBM­]?æÆ*ž[—£?ÏmBM­]?ÏK ¶ÞÝ?¿«²~u"?è-ÒH{‰?¿«²~u"?،éC½?º² Ã?ã¹ò‹^~¢?º² ÃMIXED4FGL J1844.4+1547¿æhn ‰@!DqæÍ)À8¢Ž`€sXÀ;[vý^ù@ó%~¿£™?ÿªúêí?ªÿö3á?¸¼¨½Mþ¼@/½jY:.@£‰Ê™–¿?ïæ(S`'¿âzŒŽ\¿Ù8i}òõ¿Ýx6zæP¿äXÅÉ£M¿âØ€_5ðAGNbll3FGL J1844.3+1547NVSS J184425+154646?ïû–ê®é??;bÞO)?A¥ø% ??;bÞO)?ïŒéø¬¤Ž?—(8÷¹?ŒÅÃ¨Ðˆ?—(8÷¹?ïÍ2[Øÿò?~ &€d?Î?yfÒjó?~ &€d?Î?ïÕsoÁâl?Z§æÎR¡I?uFH2W?Z§æÎR¡I?ïü/h£Wˆ?6¤"£'œ?>"ºEÕÜõ?6¤"£'œ?í80õٔ?Á%i]´¦?¶>gXá?Á%i]´¦?ï¼m‡ÔŒ?†;Ì&75ò?€äžÇnï?†;Ì&75ò?ïsì¶Í.?}+Ç:Ýè¦?''i)ÎÖH?}+Ç:Ýè¦AGN4FGL J1844.8-3248¿éõô–WÀ*)#å¸VÀ:ßT¦Ë±À<VÛÉ¿Ò@ çk $|?ýƒqÚ7ï[?ÌBûRFI?ÁJ¬ ¯Íã?÷<c'í"Ó@¸c3V?ÝØ̵O؅?Ù›ÍÀ"?ï&;Óë¤ÿ¿ÔÐ{)Ðß¿ÜöØ9™…¿ç>¢ÉAGNbcuNVSS J184445-324641?ïúû+9À?VñâÕP•¡?Dñ_1;7?VñâÕP•¡?ï¤Ëp3!?Ø¶'(iÕ?†Í#ùs7Ê?Ø¶'(iÕ?ïQþ°?"Š<úõ8®?•Ü^€·ø	?"Š<úõ8®?ïEEuó?~Ñý5ÌÄ?—\·`àÝ©?~Ñý5ÌÄ?ïîU0=à?kƚegÔù?aªê®ÅßÍ?kƚegÔù?íɅ3tæ?ÂX &H?·é³Ô>—Q?ÂX &H?îúLÃՅ?›ÙÝIjÚ? [3Íò®?›ÙÝIjÚ?î5_a©,#?žª|¹æ ?¬ª	áý¡Ü?žª|¹æ AGN4FGL J1844.9+5709?ÔþD]@ç–@7`ÿ—$tTÀ9æèˆêõ­À<pOŠL@ŸÍ¾G[@h§¤WÚ?´Jßø"»í?¦³À¿Ö͵?ñ"wXüñX?û`gô°ì¿æX¨mqób¿ÜÀff²g¿äiÿöÅÅ¿à⣘öÜk¿ãö"¡¸!¿èÖNUÎAGNbll3FGL J1844.1+5709TXS 1843+571?ïøtwîpƒ?BºÀ6ïc®?N.!9³?BºÀ6ïc®?ïÜ֘†&Ô?wY¬3šG?q"³¢ÏŽK?wY¬3šG?ïÝkÙ?pÃbOfî?qJ€Ú•Á?pÃbOfî?ï?ˆ,E—?<àŸ'N)?˜úr6#4?<àŸ'N)?ïÚ)H<ž†?jRÇîÐ?rë[×aé9?jRÇîÐ?ï>9Á­?¥Œ²ƒuV?˜8ÇÅò€?¥Œ²ƒuV?ïÅ«u±?ß¯i˜Ø?}vª/Ù¬m?ß¯i˜Ø?윁ÍÂc?§±"b°˜G?¿ëñ'ìì?§±"b°˜GAGN4FGL J1845.0+1613¿íúš<§:@!cåÙä"À9Ñ°C)J|À;‰ôRLÓî@+³Ö0Ϊ@ïsÚZT?Àñ®X˜r}?§;ýå§?é^«QR+@ç;2±A¿ïü+ഐ?ïû4SÄ£3¿èe­¤™`¿åøç¨eݿᆌáû2;¿â‡¹1åUZAGNbcu87GB 184225.9+161105?ïï*K>S?Z
?c¯0;?`Õ´ŽÒÀ&?Z
?c¯0;?ï˜Ô¹;†¥?"ç=Ã-\r?‰ÊÑ£_æÑ?"ç=Ã-\r?ïŠã`'?…Rª5·á?G'ܽۘ?…Rª5·á?ï²ÆIX—#?gñÖ\C¨ñ?ƒNmÓ•2?gñÖ\C¨ñ?ï8ž÷d…?"ÍûEèì?˜ì! Ã[?"ÍûEèì?ìù³Ú&kh?¾ÙŸ-­7[?¸2a0òf9?¾ÙŸ-­7[?í§¥
ý"?¥VY¶§2?²Âתœ,c?¥VY¶§2?í»¹÷Ýò? ÑøŽOA9?²"0@¢x	? ÑøŽOA9AGN4FGL J1846.7+7238¿ï ¾#Å5@:%9C¬ÅÀ;r«¯EÓIÀ<õøٛi@!‡Ý^?{k?ó|tðlå?ßÀç,¬0?َޖxÓ?ÿ›x¦@ÿm[M-°?í[Ý¡[Z¿îñÄhz<Ý¿Ñç3À̹W?Ú¶ÁÚUv¿Î0¥å,j¿åÐîš|îhAGNbcuRX J1846.1+7237?ïýçd'ÇÅ?%ì•`|¹–?0ÄÞ+Äm?%ì•`|¹–?ïöé(?Tþ+¹G,?Sü-æ×µÀ?Tþ+¹G,?ïї{‰›?r,Í¿l6<?w4Bgܚº?r,Í¿l6<?ïüq¶â¼?+æ¨ó%??q·Çn©?+æ¨ó%?ïþ¡8Ir?%Â'â¹Ò3?%ìy÷glp?%Â'â¹Ò3?ïÐûxºY‹?'cg½u'?w'CÁÊ6?'cg½u'?ïê×.`Í?qÇä«ځ?eí("Æ;¦?qÇä«ځ?ïùHÌ^?CG S(-?Jßû¥•·Ë?CG S(-AGN4FGL J1847.6+5219?ï¿T•>Ò4@5¶–6—lÀ:ñXeò£ À<¾ÿ
6º§@ljßgY+?ÿ̀CRe?Ðc"GÁ`?Ð	ZÝN@XCùTT@z$'±rÿ?ÛT9}¥Z¿á*¥Å÷Æv¿â&©ý¿ÞÓ¿àÐ×ôH;Ù¿é¦n£KÊ¿ïÿþÞ÷AGNbcuNVSS J184754+521513?ïéåšÔ=?_c-"Ï?fóŠGŠb?_c-"Ï?ïé«Xš7?fõ** 8?fT§Zû×?fõ** 8?ïÄ䰐£s?tžà3¨Ã?}§œ1f?tžà3¨Ã?ï¶x#ʁæ?]iâµ'ý¾?'a÷Àž}?]iâµ'ý¾?ï¿ß€¥ú?zŒÒ;l¬Â?€Ê"àï?zŒÒ;l¬Â?òd¯?9‹o'èƒ?ˆÕƒ††6?9‹o'èƒ?î¢k§eV"?šyUòÉãC?¥ÙEŒ>KÇ?šyUòÉãC?îÐÀòEy©?ƒô›jKš«?¢óðßh?ƒô›jKš«AGN4FGL J1848.1-4230¿¯Öâ«TƒÅÀ1_󾩛À:Sˆs©À<(ôB\›â@Ä:P]æe@‡zÛ?¿e')]œh?«$|a$ˆ ?îVužèŽ@ø`ÍöŸ?ïöðÂuZö?ÓÒ)-ó»¿é¡¿ØȄ¿á|×­O¿æEòèn¿ÕÏ°¬AGNbcu3FGL J1848.1-4230PMN J1848-4230?ïò¼(ËâR?r'¢,ËE$?Z‡®ÈpjÎ?r'¢,ËE$?ïâ׏Ϫ?sæpÒC
ï?m(põQ'?sæpÒC
ï?ï¯{&M,ë?†yH]•F?"!6y]D?†yH]•F?ïßϺVl?T{ŸE›?pw2¢ý¹?T{ŸE›?ïÙ·`܄?w+=²qc'?s$O×äñò?w+=²qc'?ï ·n|ñ~?"Æ5«sæÌ?‡Ò$VtÌs?"Æ5«sæÌ?ï'Ià¶?»Û
pC?m‡Õ½Zk?»Û
pC?ï>kJ¦ÂL?"<²,`?˜2–«'¶}?"<²,`AGN4FGL J1848.4+3217?æCò{»•Ë@-_r'Ä"BÀ8'ÞѲÛÀ;il«$@#åÓ©‹@B[úҙ•?®(~îÙ£?Ç5Z«'@ó<£~@ŠÂ'4›¿ã'—|ˆç›¿Ùl`üD3·¿â¤«ã¢Ò¿ç皮l¿èʾ­	c¿ðAGNFSRQ3FGL J1848.4+3216B2 1846+32A?ïi¹"=l?"ç}øàCP?'ÈÏs7ˆ—?"ç}øàCP?ïÔ
¯|@)?†¨à¤ê?uù(W-'?†¨à¤ê?ìދl÷?¨n&¶)?¹¤ :ð?¨n&¶)?ïú£|ÇPâ?7Y,Éç&?Erœ^<?7Y,Éç&?ìîó",Ü?²gDé±7…?¸ˆcßí?²gDé±7…?ï 0%{~?«iÑ…6?ž+ù÷àô7?«iÑ…6?èÉZ=§ð
?²Dk"|^È?Ìڗ	`?Ë?²Dk"|^È?ïáDHY`?dIª2º?n»·Þù?dIª2ºAGN4FGL J1848.5+6537¿²ªÖ©€¨˜@8Õã§Ú¤ýÀ;1CºióºÀ<Ú!›[:¹@!'³­Áð?øçKƒŒ?Î2Sº<Qj?ÆÈdȬ©?ûõÓ £äv@ö{¬ô•>¿çW>«6z¿í²1«s¶±¿Ì"Æv)¿Á!JÓbé¿Üà4óý">¿Áº†ú¾VAGNbllNVSS J184822+653702?ïÿ	ÿ÷á<?$sՆ1ª?¿üƒŽ­Š?$sՆ1ª?ïö.TžŠ<?VÆÀ9²¦u?S£VOx©V?VÆÀ9²¦u?ïñøxÕ²W?dVG"þý?\
ØébE?dVG"þý?ïü›UÃø?%'/nƒÀ?;%Vûχ?%'/nƒÀ?ïÿ~|vŒé?;ß͍ªÓ?0oÌWïû?;ß͍ªÓ?ïͦÝ,žø?€¨‡.B©?y,'b!`?€¨‡.B©?ïï"2&˜Æ?l%êE'®6?`kÍ¿J2?l%êE'®6?ïõcx±V?HùYs+e?U9Ù t?HùYs+eAGN4FGL J1848.5+3243?íÍíc¿'@-¦¥.ùÏÀ8oSö!YíÀ;®»iÎ@hé‡B©ô@ß=?%°?¨iäöd?º˜»Î!á|@`ÔV.@¨ê×ÿ?ÝN;Í5¨¿ã9€hÆ¿æ‡Íôêù¿å';C¢ìÿ¿èÐÀ⳾߿ïþ¶ôô3CAGNfsrq2FGL J1848.6+3241B2 1846+32B?ïíC	ŽÌ?b=(΂
õ?b¼÷.*£Ø?b=(΂
õ?ïàã•8Ù?|7tý€8h?oá"v•?|7tý€8h?ïq±ôŒâÛ?ai]ƒí?'ÉÁjô´?ai]ƒí?ïúÜ©tê?4ž£'Äh?GàŒ3t?4ž£'Äh?ïèµ&¤Ù?cŽ"»Ü§›?gJِ%6Ñ?cŽ"»Ü§›?ïm,pÌEé?ŸVÚ¾c8Æ?'Zqä¿tÚ?ŸVÚ¾c8Æ?îãÜ?ÓÌé?›Â"©^¢g?¡Â</|z?›Â"©^¢g?ïá²mX¦"?aöÈÔ±¦ã?nM'Š|µN?aöÈÔ±¦ãAGN4FGL J1848.6-2711¿ÎRì3MÀ&é§~^ª°À9éà¸<À;¹á`x@_ß4ÿ@S{š«'?ÊÀ	šÞ?ÓÈ5Ä+m@OÀ1³×@ÂMò§'¿Ì"ö%j¿â¼è‹+B¿è±`Ëò¥¿êétšпïþظ"Yä¿î…§ß­z!AGNbcuPMN J1848-2718?ï?¡œOçb¿?œ_ÄQ–?¡œOçb¿?íÞèàœ?·ÞÁ"kËZ?±¸þÕ+Ã?·ÞÁ"kËZ?íC»V,ÝY?¢µ³bä†?µâ%LáG=?¢µ³bä†?î2Ý?zÐ?›Þ ñ¾?¬Ò/~œö?›Þ ñ¾?í.®ò¤Ö?²º¬½!ƒê?·nŠ‡üåÏ?²º¬½!ƒê?â­Xñ¼N?ÑêóС?Ú¥N‡cü?ÑêóС?äýãÏÚb?µX¦EÁa?Ö9Ø`K<?µX¦EÁa?ã¯æÚa'?¸÷Cš"?Ùî 2K<û?¸÷Cš"AGN4FGL J1848.9+4247¿ïÿ¤cÞ2@2wiDg8À:"~ù˜À<…uôxãA@ 2N@CRë__?ºÜdÅQƒU¿{^^ÞßS?½õc|@ê#sw›î¿ï꽟ˆF?ïÿ–þߙƒ¿à&D7guZ¿â0"!'÷¿¿Ü6^`Þg)¿ÔÄʟËãAGNbll3FGL J1848.9+4247RGB J1848+427?ïý»Ñ
4'?(ïó©î™?2!wìϯ?(ïó©î™?ïïÈ=#ªˆ?gŠ°ÔèßÜ?`7Ã0ð?gŠ°ÔèßÜ?ïóØRD£ü?K/ï€dá?XO[4¿‡b?K/ï€dá?ï÷¼H<É?7SˆÔJËÉ?P‡ḯ?7SˆÔJËÉ?ïøž±Óą?HÐI,AJÚ?M…8ÆëkY?HÐI,AJÚ?ïµÝ¸é|A?ŠÂyBÔ>p?'ˆ'¸êaÇ?ŠÂyBÔ>p?ïìä^'ÂV?moè[LÆ?c¡ã<j\?moè[LÆ?ïæ
ðbÂÝ?\Xl"öù"?iõØVk?\Xl"öù"AGN4FGL J1849.2-1647?Ø«®@çôÀdkA—zÀ9Ä/µÐ1À;áRƒZ'ô@! •ÀR–?ÿ³LØç?³Óc"ÏÛJ¿¡t=‹Yn?猪Œžß?Ø0=³Gs:?ïЍa'^¿»YÓ0C)¿åè°;Ä|¿à¿…òèn¿Ø=ÏCtžã¿ËpÀ•ÆAGNbcu3FGL J1849.3-16451RXS J184919.7-164726?ïÑ´:"¶3?ÌƧ|?w%âÌB–?ÌƧ|?ä.¡aÎ×?Ð:ZѪ#¢?×¢½=ÒbR?Ð:ZѪ#¢?îÙø§?›ë"µì<}?¢`sÒ‹ù?›ë"µì<}?è5ž/Þót?³ÂÄÙ_î'?Ï)‡@"22?³ÂÄÙ_î'?ï‰PV3?•ÇÌ1ò@z?«êc'tØ?•ÇÌ1ò@z?ÆŒ…ÆS?Ë1€M?ê{\ގ|k?Ë1€M?ï¢j£Œâ?"£öƒ™A?œk²«Žc°?"£öƒ™A?Ï~W|qHJ?·	KWÕœ?è j ã­í?·	KWÕœMIXED4FGL J1849.2+6705¿ïØÙ÷òY=@9
ǸÕ¦À7×Øã["‹À;"1ί%@mvK½Ä@Äù¯"?"œÃ"\©Ø?¸'t·7_@""ÇSçá@EŽŠ$¿Êƒ]Âþ¾¿à.ë¥Õçÿ¿ä»ð¶ù&¿äâ1ƒ/ÊÉ¿è	}WC´¿é%¥á¦x¥AGNFSRQ3FGL J1849.2+6705S4 1849+67?ïø^.š®S?Hé蚋Á?N‡EÖU•?Hé蚋Á?ïÙ&xÿ_
?‰‡Ä­ã?slÃnrƒ?‰‡Ä­ã?ï¥÷†'^o?C»Ÿ0ó?†'Q.?C»Ÿ0ó?ï÷=Þª<L?Kb…Ø7¿?Q"C;Øn?Kb…Ø7¿?ïïx#?ZîüÉQ´?`ÿbeÄÈ?ZîüÉQ´?ïD\ëW?°ºNph'Q?—·Ò1?°ºNph'Q?ï©Þûù`)?‹Îq>eÿ)?…ˆAfeÀ?‹Îq>eÿ)?ïņ@,Í?ruz‡x¥?}<ß³Êp?ruz‡x¥AGN4FGL J1849.3-6447¿ãøGÅ•ÏÀ8&A€ÓÏöÀ;+–^{¶À<¼…"êÔ@ æõ'çôp?ûyüE`\a?Ð˜'\?Ï||¨G1m@BؤU@wHÐöR?½ðÊ1u?ïãNÿl‡=¿åÊÁžpn¿»¼$^@|¿Úœ=£N¤(¿ïÿú Âî'AGNbcu1RXS J184924.8-644933?ïùûnW,?Ap)‰áæ?HGÄ,L'?Ap)‰áæ?ïäŠw¡f?p7Y¿Ù.8?kuóT$ŠC?p7Y¿Ù.8?ïÉß­5i?s
Ê}×?{x5Ãão?s
Ê}×?ïÚ®a…?ZWa/¸%?rö¨à«É>?ZWa/¸%?ïú]ŽÑi•?B U´oËá?F‰Ägã?B U´oËá?ï—?ŠÚ?—â.Ÿ)ðL?Š0YK-¢?—â.Ÿ)ðL?ï½je	Ö)?-Øo1*?€¥f°{ñÞ?-Øo1*?ï@ÈfØôp?‰â;Œ²[?—æó&™@?‰â;Œ²[AGN4FGL J1849.4+2745?ѽZ*»6ð@)U'Í}åÀ9÷ö•3À<&/Ta"@^dŠ$\@¾‡Ó[?½pÛ	{~Ñ?ÀÀç¦ÂÌï@Ü \–ÙÌ@e£zîޚ¿à«Ç>B…â¿ÚC¦³]þ¿áô.`:¨H¿ç
áŒR3¿ä•îê.¿ë¬ížÔkýAGNbll3FGL J1849.5+2751MG2 J184929+2748?ïü2.a£o?;$zzâ9)?>nŒ'	@?;$zzâ9)?ïßAh¢x2?u­'¤um?p_K®û?u­'¤um?ïçGŒÜqÛ?ib"ý'2?h¸sS¨¬Y?ib"ý'2?ïîßQ'L|?CGéÊÚKý?a ®2š<p?CGéÊÚKý?ïӄÎþ¢ª?zÁéÛqí?v=˜'ܶÐ?zÁéÛqí?ï6«Uâ=U?¨•Éµ©
I?™*•>ëg?¨•Éµ©
I?ïj(oฒ?'G¯é~?'ºòX‰»?'G¯é~?ï³båÊÁý?n†^W'õÖ?ƒ'F—F^°?n†^W'õÖAGN4FGL J1849.4-4313?às
Í·ÈÀ1ÛV†''À9BT^üå™À;Û[Z™ª@Ú`	]L@úéZ¢
?­	*ÃoxU?½[3­VÚ@Kèÿ2z§@¢ç÷ ?ïÿã°> Í¿ÙAf|·¿âÃ{_œÈ£¿âAb ß9¿é'´þyî¿ÑM`pƒÛAGNbll3FGL J1849.4-4312PMN J1849-4314?ïú¼"]".?A£b–?E
²ÿ•ó?A£b–?ïèζÞ?u,´òÆ©?g1IåVzn?u,´òÆ©?ï¯Ú¶øØ¢?~©ƒ<MÅ?"	RD‰‡?~©ƒ<MÅ?ïèØѽÍV?MÔúRÔ±x?g'."º?MÔúRÔ±x?ïõœ©d'?Xâ,HF
?Tƭ฻î?Xâ,HF
?]<¢?œLýi	ÊR?‰è£<ç"?œLýi	ÊR?íóöŠ
…j?£''¤‡ß2?°`K¯«Ô°?£''¤‡ß2?ï‡àWªG"?wG<w¦þ?ŽêŽÿ†?wG<w¦þAGN4FGL J1850.1-0758?ë<»êý9|À
½œtÜÀ9£Y7©ºyÀ;p]j>b;@'"ß @!ñÂO›I?¹f¢vb¿Ÿ 6^êNÆ?æ§VPn­]@羊êª-?퓢¿]"›¿è^ï^Èt¿ç}1¦¿ó¿ä¯'Á8¿ã€!ß&¡¿'
©¥š»AGNbcuNVSS J185002-075842?ïïÕÔÁ?Xø<þhD?`ù*;þ^ñ?Xø<þhD?ïµñ`w?¢ò̊Â?)<¬‡?¢ò̊Â?ï­ö£4øÛ?BQQŠðâ?"'W2ÁÉ9?BQQŠðâ?ïÉÆZöNY?_(´Q]?{҈ø[w?_(´Q]?ït*Ÿ:î>?Š<½Ô?'z¬zÎV?Š<½Ô?í`'–
?¾Ïè©)ã?´ûƒîu2?¾Ïè©)ã?ïv¼Ûú?˜øҜì÷?Ÿ¾'(d€¼?˜øҜì÷?YÕ*â?'OÿáeúÊ?¦TJaÑjç?'OÿáeúÊAGN4FGL J1850.5+2631?îüµ}zÕ@'ÛeDþ6ÒÀ:¹ß[DÊ4À<bèn@"¾×M.\	?ú'ðßьO?ÄÃô÷cNY?«ˆã$8U?çF߂±öˆ@ªöŽ<C¿ì3q|D=?ïϤîar¿Õ—"{ªñ0¿ØGt^4¿¿Þ²qA`Èm¿Y7ÕÀwAGNbllNVSS J185023+263151?ïûùK†?8Ë´vÙöÀ?@Ñî0Kp?8Ë´vÙöÀ?ïÊ_nÇÖ:?–
W¿&†?zÐHœâÕ?–
W¿&†?ïç"upÍü?o¯k~ë?hlŠ»-Ã?o¯k~ë?ïÊß":p?eSYâ~À?zx"àGÓ?eSYâ~À?ïóƒh³É?S9É3<þÆ?Xøå9—.½?S9É3<þÆ?…¥?¨H…°J?œcÐf?¨H…°J?ïèfY-÷=?tß·P[?g™¦ª-Kw?tß·P[?ï;‰9åC?‹'=Nð?˜Žß}êÁž?‹'=NðAGN4FGL J1851.5+3406?Ø@ýSÛÒØ@-šÀY!À:;ţàÀ<n}'Þ[@@+0Û?+@Ÿ¼?ÈU…2à'?¹'8©ê ?ïf='u^@vwŽ
?Мöÿn5¿ëäa>y¿šW'Yb¿èÅŸ,«…¿Øò»ÈB¤¿ïõ‰ŸP'ÀAGNbcuB2 1849+34?ïþ,Xx'
?(¨@'ÇÈ?-:v×A¤ï?(¨@'ÇÈ?ïéaüQþ-?mTîRLU?fž¬¡úâ?mTîRLU?ïëݼîÄ?it<
ÇØ?d"ù~*ƒ.?it<
ÇØ?ïõ¨ã…î8?:AÈé¢Ï?T®9^ÞÓ?:AÈé¢Ï?ïü˜'h?=ÿ"t.þ??k=$¹ç<?=ÿ"t.þ?ïšÂÃ"mØ?'‡²2äü?‰OO>CÁþ?'‡²2äü?ïèԄž'.?rÆQ^"X?g+{œ—ž?rÆQ^"X?ïڎÊï¹?a}OÀÇE?r¸šª‰½?a}OÀÇEAGN4FGL J1852.4+4856¿ïò)̓R>@3òÜ]cˆfÀ8ä
kùMÀ<+ÑÁÿq@±à<Á&{@ï"b*˜?£&b•K3?ª†·>Æm@à5z5PD@&NIºO¿½6‰©âg¿áŽ­½gÿï¿å§|æÛkÌ¿áõÁb¶Y¿å U—¿ìÝ5Мe&AGNfsrq3FGL J1852.4+4856S4 1851+48?ïþ'hçŽß?¾5ØU?&Ùoçt‰.?¾5ØU?ïò\ä?bõU'\äÕ?[÷EôçU2?bõU'\äÕ?ïôª—ß?`çÿÆ-Ó ?VªÑxKÌÍ?`çÿÆ-Ó ?ïÿnG°ª?f¡´cIG?<ñkPç?f¡´cIG?ïþK ùp€?"ö_ɘ/?+EïF²›?"ö_ɘ/?ïÇ—rwí?ƒÂª·­Ê?|x´U2eœ?ƒÂª·­Ê?ïä¢
g?v6°)|ö?kì]çáØý?v6°)|ö?ïÿTÝ/¤?
AHtdsF?d^QIJÖ?
AHtdsFAGN4FGL J1853.8+6714¿íç¥×¦«·@8£NÛʗÀ;@8
‡=À<OìTR@ z}l@($¹ó¬5?Ò¥Y€ÏÉ,?Çrç~(úË?óµZ¥hõ@‹ÒªÝ8Ö?Ò/£#Ü¿íheå7&Þ?Û5ÚØS>¿ÜóA«›ú¿ã€;ÄÒ,ˆ¿âùZ"¡UAGNbll1ES 1853+671?ïõÅ Cèô?R.CBo?Tt¿Å%W3?R.CBo?ïìbÆu?b…p½6gª?cäž5ÊÛ?b…p½6gª?ïä}:"NÒ?lA§Éì9?k'Å",Î?lA§Éì9?ï¶ O£"Ò?fÄÿNV\?'wì!.)…?fÄÿNV\?ïô<r¢ÿ?V	1Ñ
(‹?W‡ä×?V	1Ñ
(‹?ï°)9E'&?ˆÞuÛh4á?ƒõ± áw?ˆÞuÛh4á?ïwoŠsÙ8?'‹>"âÁ?'¶¬B÷?'‹>"âÁ?îè'ÇZ?"Ï	¬Àא?¨}"jQe?"Ï	¬ÀאAGN4FGL J1854.6-6007¿îÏePð;À7®Ý&·#îÀ:åùrGEÀ<¥¸	â@ù&
s±?ýâEîÑ?Ðd!s€?Ñ3©$Ññz?û¯É†Ç.þ@ÖQ·'¸­?înkón!¿ì·¹ª±?âP¤'ñ߬¿äqÎly¿àNQ!/Ð}¿ïþ\ÓAGNbll3FGL J1855.1-6008PMN J1854-6009?ïøÜ`FDf??Ð}$jO?LŽ‰øÒ??Ð}$jO?ïìäW­ç?f_鼨?c橱ñ&?f_鼨?ïµ$Sé®|?{›‰Åâ?'¶ëÂlÕ?{›‰Åâ?ï¼ë…tŸ?iœüýx…ˆ?€üàf?iœüýx…ˆ?ïôðZ.—?R8›1>ÿ?Vòî-re?R8›1>ÿ?ïÅ]!™,â?€ž»œ?½?}Qo4Éfã?€ž»œ?½?ïuÝ$¼U?Ž«ڍ?'D[f½€'?Ž«ڍ?ï5!µ\m¿?ŒÃN»þ2?™[É]	N?ŒÃN»þ2AGN4FGL J1855.8-2028¿è‰%µUÀ$<âó¾ýÀ:ÍËÕVJÀ<>¥}Ójv@8£ÆCEÐ?ü{"¤£?Ô%ߙX+?ÝÎÆâ}
G@¦ò¥¤i×@	%rÒ/6¿éŠ"XŸÔ?ä¸Q€%TM?î¾h›Œ¹¿ÐDHÄ¿ã¿éåBnºs¿ïüHOúêAGNbcuPMN J1855-2027?ïùž•½þ?MP}à½?I…¨	Ï>?MP}à½?ï˜éU)?"Ó_ÃG?‰Åª±©a·?"Ó_ÃG?îÈ«Îá‹1?"Í/x\•Õ?£uC/~ò?"Í/x\•Õ?ïëm ê±?w"¨—Mþ?‹Å$´U·¶?w"¨—Mþ?ïîˆL¦]?b£'§ò?aw³y?`+?b£'§ò?îTqz?¼oÿ	"…6?¯ŸíL]?¼oÿ	"…6?î"þ"Á\<?4rð¯ÍZ?­ÐϞ¹>?4rð¯ÍZ?ï9Ššo¤Ë?'þÂÛ_Ì>?˜Î¬·2Л?'þÂÛ_Ì>AGN4FGL J1857.9+0313c?ÙD*Ñ(ÀØ?$yςgÀ8€Ä0FéÀ9É瀭9Š@󾑠¦Ô@oÃzn?Ô¨(÷?ф(£ãž@	oŽÀøƒ4@ˆLôzeÍ?ïM›^•·¿ìMè@EÀT¿áÁcâþ¿çª.£ˆ0¿è°KŒÆL€¿á_#a.AAGNbcuLQAC 284+003?ÞA¡Ñݔ?Ô×ñ­pªÒ?àß/6?Ô×ñ­pªÒ?àØzç
&?ÐÊâCxòý?ßöO
1å´?ÐÊâCxòý?݋ R‡s?µ"%6Qh?á:/ñV¼G?µ"%6Qh?赊¯'f?¯7KöÂw?Í)ÕA÷'i?¯7KöÂw?Ø´iÂDY?Ó­P±¯v6?ã¥ËÝ÷Ô?Ó­P±¯v6?´=ÒQÿ£¥?À‡{?íxEµÛˆk?À‡{?ÚVÙÙz°?¹{äuŸ3?âÔý"B¨?¹{äuŸ3?¾ÕWÓÚß?¯4Þ%‡?ì%U"¾?¯4Þ%‡<MIXED4FGL J1858.1-1821¿º¢LŠaDÀ#]FÞ	5À;¯¥t™/À<)ñTk'@ v‡¬‡2@
 >ÏH¨?ÌǺ.d—?–î$"æ°?Ð"g~>tZ?þ6ÍVWP?Õ_"¥Fv?ïÈ!‡¿¿èxpT%ò¿Ýùu3ܦ¿Ý¤çá%If¿åŽx¾­¥?AGNbcuNVSS J185806-182314?ïùM$\;ü?FýÆWþDÅ?JËn^¯(Ú?FýÆWþDÅ?€CB†?'ò]Àw?ˆÞŸï/^y?'ò]Àw?ïÙ:˜N¸?qÕåí]¥?syⓌP?qÕåí]¥?ïÎPéãš*?b̨Ë´?x׋Q2ñ?b̨Ë´?ïô¼H¬Rj?Y—t«Äƒ™?V‡n§[+Ó?Y—t«Äƒ™?í‹«*2%?½OS‡3?³§Z§bW?½OS‡3?ïµ(ð}ðµ?†æeÇ|xC?'µÃë*œ"?†æeÇ|xC?îÏk%p…'?–®÷ÈО&?£	M«‹\á?–®÷ÈО&AGN4FGL J1858.1+7318¿çØòr×@¢@9k©Ÿ¡—À:qt4…BÊÀ<{Tç4@ôœDCѼ@…w£¥Œ?²{"O…y¿¶lþ[EB@E–È.›@_ûé
¿áˆØÖ+¿ãMMüUy¿íMÖýÓ*	¿ÁÔüÇuC¿Ú{"BšY¿èê–o AGNbcu3FGL J1857.9+7319GALEXASC J185820.26+731714.3?ïøÍ¢›Üü?DŒ+øǖÁ?LÉt"'?DŒ+øǖÁ?ïÝH
Æù4?ruNXÏ	H?q[ù"iÔ?ruNXÏ	H?ïÇ }Æ?|Ã[ûL"·?|/ÁeoÙG?|Ã[ûL"·?ïÞÅx£2}?X^/΋Q?pC8µ~?X^/΋Q?ïÂK[	?x[<ë±}?~ÚRsί?x[<ë±}?î£2±Ði‡?ª™h'xî=?¥ÌÔâ€"?ª™h'xî=?îã5k5œß?—»ºZù-¥?¡Ì©J}?—»ºZù-¥?íö:gb˜Y?¡+‰Þ Ô?°N,ÅY0¶?¡+‰Þ ÔAGN4FGL J1858.3-2511¿À/ÿ
À)6~À¨À9!áKßÒcÀ;§5Þ^s@ÈWC"?@µ»8OÓ?±¸põ5¡¢?ÉX"*ø&@e8}@6sšœ³?ïü··ïÆ¿ßÞT~ÝU±¿åN¾Ôçx¿ä!H2ž¹¿êª¡Ô¦‹¿ïÿCAž0AGNbcu3FGL J1858.4-2509PMN J1858-2511?î"Bð?µ2²ÿ£*?¦¾ÛӒô?µ2²ÿ£*?ïZÕÿP'¤?£Z‹ËQæ?"¥@7Ýv?£Z‹ËQæ?ît''9(?š?Ë9REÃ?¨¶æß3°?š?Ë9REÃ?ïtXzsV?sυ)x1?'tð¸|m@?sυ)x1?è•
\Ȕ?ÇÄÄÄÚSã?ͫˆŒÝ°?ÇÄÄÄÚSã?ì´Q«Ä>‰?Á®;^<?º]r¡Þ¹?Á®;^<?榦øì?½ñ'Vår"?Óø³Â²'?½ñ'Vår"?쌜N»àý?¡‰ªÿ–¥S?»›Š ø?¡‰ªÿ–¥SAGN4FGL J1858.3+4321¿×"zŸ>°@1>ž¡À:±Ðz×6³À<‡©qÛ@…z±!@›¹!]¹?ºH¦7Û?±¦ÿ!¢€ã?ïÁŠ¿66H@Ö%f
?í}Zi"?АC¯'9+¿èqÿ¡¶I¿ÛÔS±Wü¿ã€§û\,Q¿ïÿÿÊPËAGNbllNVSS J185813+432452?ï÷ô;%›?EÌˍ‡?PÖ
_k?EÌˍ‡?ïÖdbwÓ?|‹ ×V`°?tÍÎÂ'Ò·?|‹ ×V`°?ïãËNr~Î?dŒ×<[Ð?l4±2p?dŒ×<[Ð?®Ló½?l~µÓU?‹ÓÔeãد?l~µÓU?ïåßLp
?c	(GÇ¿È?jü ¶O¦?c	(GÇ¿È?ï>¾s»? ±ºÁ•2Ã?˜(1€V™? ±ºÁ•2Ã?ïÉw®?÷o?JèÀû»?{D(èCX??JèÀû»?íì¹ö ³?–Õz)}Y?°š0IG<m?–Õz)}YAGN4FGL J1858.5+0640¿Ù…ìFBb.?÷øZðŸÀ9›=EÀ:…õ|ï>è@ ºu\M‰@F49Ãp-?Àå13ûÛ¿EłVž@[?çK©!?Çæ{Ÿˆœ?înÊî¦;i¿ì.KlåÜ¿å
ÃþGB¿áqüfîK£¿á®M?ùÀ AGNbcuNVSS J185831+064016?é°ù$͆?ÇêvxN½ ?É<lˍæ?ÇêvxN½ ?ï5¿e8Çz?«+Wˆ_´?™HUwt¹?«+Wˆ_´?æùAú>ü?´¡—u?Ò
|á'?´¡—u?ïy_]L{?yC€ŸðD?Þ5¨"?yC€ŸðD?ã.ùžÝŒ?ÎEB[€k?Ù¢
ÄÂDç?ÎEB[€k?ë*Ê
L;9?Å4ýÿ…íÑ?ÃT×ÊÏ?Å4ýÿ…íÑ?è8;õhf?·"åüYég?ϓ*^g?·"åüYég?ì'Ñ!EJ?­­Ô­?¾ÇvõÕ°?­­Ô­AGN4FGL J1858.7+5708?è‰yL¶Ö°@5Ìÿ!³¯À:Æ÷–¤ò"À<¥¼ä!}(@ƒ¹ügÅ@ÉYø™Ú?DZ~è"Q×?ΫúÅ-œ@à f§ÔÆ@oüt°++?ïòæ§ieõ¿ÞF~1ß ¿âxP©e¿w¿Þµã¼¨gh¿ïñIï7Zà¿ìY? (ªAGNfsrq87GB 185759.9+570427?ïÉZÈ´ l?w ¹z1äÇ?{R›²Ió?w ¹z1äÇ?ïÔùÛ½oQ?{S'«3É?uƒÙûÏ?{S'«3É?ïv‡" ê?…ùBd´?'/u†I?…ùBd´?ï4âá>ÒV?vó˜ÚÆÄ?™c£ßí,?vó˜ÚÆÄ?îì)ÉI÷?›àêõåq?¡=cj‹ù™?›àêõåq?ïcÈÍlb‡?";×Ãd?"†æMLE?";×Ãd?íÑC»&î?¦ïcº4zÎ?·ÉuäLŠ?¦ïcº4zÎ?ì—.Eô½? i²_ÞîÖ?»FÐZp? i²_ÞîÖAGN4FGL J1859.0+2329¿À™-ý®@!ÉdobÀ:M¼àÆ~ÕÀ;á<aNÏ@F×zzÅn@ã `ȗ´?Á,C܄¿€fX¤†Ý?À§H®ÅzÉ@Õ;@ráÊ?ïÿŸR@>´¿ßqªgG7¿èí5" ¼8¿à¨>b'D¶¿á¡HÌ!¬¿Ý¤ëGWAGNbcuNVSS J185857+233007?ïíìôyRì?a¶'¢KÕ?bhp"0?a¶'¢KÕ?ï¼#Ü vÐ?™r…R$ª?€÷Ú¡ü?™r…R$ª?￘ÖÈp"?}(%ü£?€ÊK|!?}(%ü£?ïÜ…-¯n?Q Š´ÒÅ?qý=5Œ¹?Q Š´ÒÅ?鹿ežî?†ð#š+?†Ÿæ¦ôq?†ð#š+?îõOd}i?©
X[ `? ¯KÞh?©
X[ `?ï•eq7¿?–þ%&®?ŸÍSIB?–þ%&®?ï%&PÝÏ:?"+UÂtò*?›[5àÖ|Ë?"+UÂtò*AGN4FGL J1901.7-5140?냗»·ÀeÀ6{þ;â
À;FÔánDÀ<µgÓMðN@nl <K
@è"úô'…?ÓÁi¢#?ãgþFÂ\@
0¡C§?ó ·?ïE´À¦Á¿×Ñ¡³CŽË¿Ñ¬ÿuìk¿äbÆÜ	¿íÇ4—ɶ¿ïó_2•AGNbcuPMN J1901-5138?ãa	;#RÒ?ÐrfGeLé?Ù=퉹Z]?ÐrfGeLé?â¼ÅB¿Ã$?ËB)Gnu÷?چuz€y¸?ËB)Gnu÷?êÏüàõ–?«Ø×æêü?ÄÀÀ)¦?«Ø×æêü?â?gºç¿?®Í·?ˆ0Z?ہ1úŠ0?®Í·?ˆ0Z?Ýdn`þ?͟€8t¡?áxøMÈρ?͟€8t¡?ǧ÷çhì?ʯD,;œ?ê9%Å?ʯD,;œ?ÙØò'­Í?ÃPšÿ0?ãr"†ì)?ÃPšÿ0?·Îð°°?œ±`š´?í=¦m
?œ±`š´MIXED4FGL J1902.4-0629¿ïȨÀŒ°À‡â`²È?À:Î-À,«ZÀ<sY"ð@!¬Ê†?ÿ4«ˆ¯fŠ?ÇSŠI{õ?@àWt7?˜4éÊßb@%'}?ÚµŠ;Þ§¿æ w~瑟¿ëB1}Ñg?§­?·T¿âøô=Te¿Ñ¸#@¡ÜAGNbcuNVSS J190223-062850?ïùûÔ½Þ?EÕ²¥°?H¯Bߓ£?EÕ²¥°?ïµÇ=§çv?ÝäEf?'Ž0"Ø'?ÝäEf?ïÓ\)Ý°?x+ɃSs{?vwÑÒSø
?x+ɃSs{?ïífq	hÆ?I¿À?b™r²&?I¿À?ï믒¾?ie'7±(?dPn2ZÁ¨?ie'7±(?î*†ˆ½Ó?¼<úåcÇ?­W—wžÌ?¼<úåcÇ?ï°l—È?‡iêÎl>€?ƒûºU»Æ-?‡iêÎl>€?.Aíò?{Ihíö‹?‰\4}Bó[?{Ihíö‹AGN4FGL J1902.9-6748?àX¼SF½ÃÀ:$咖pÀ8ðÜùjº‰À;ù$(Ô4 @¥Tƒ™@¿æ4|ß?¦O§!wþ?ÀǃwCXo@*Y:-ù8@‡)ÜÈBy?¯åµüÑ¢J¿à›NÛ/f¿ç')oe©¿è.¨>Íñ¿æHp¡þ—ö¿ïÿÿ^ðP`AGNfsrq3FGL J1902.9-6745PMN J1903-6749?ïû؂ÚÝ©?9¥–Æiê?@õ´?9¥–Æiê?ïñ¬Èüé?iPÁã^{?\¦oŠŽN6?iPÁã^{?ïÍu˜wI|?zÏ Ve&?yE3¼ÌØ?zÏ Ve&?ïþ©t^? p³-0›?'åeÍ8%? p³-0›?ïýÞ(Pw?/ÈÜ€q?1¾÷|¼ø?/ÈÜ€q?ïÎKWlM†?…À=·ìL?xÚTE	Èù?…À=·ìL?ïŲÝôxŸ?[2]ý?}&êFÐâ?[2]ý?ïúXã4Üð?9ëþ?FœsbùA¿?9ëþAGN4FGL J1903.2+5540¿ÚrKþAu'@4ˆäC‹À7òË/=ÛÀ;oáÔï@gÙØù×?ý+¡nz1?™(Aà ü?µpþÅÃC6@RP.ì|•@öfÏÿ?ïý& Ñì¿×«$˜Æ5¿Ü#Q©ß¿ÜK3o™¿âê+íĔ¿ã…]7»ÄAGNbll3FGL J1903.2+5541TXS 1902+556?ïôƏà¢?wµ|ƒÉ²?Vrßÿƒ%2?wµ|ƒÉ²?îXËô?±^¬9­–i?¦/þJs@¿?±^¬9­–i?ïi%K'Ï?"KºÙÿ<?'Þ;]nÞ?"KºÙÿ<?îr{iûÓ?QwÐP?¨ØI^—×?QwÐP?ïªU
b(?'¤ü4Ÿ¯?…j½Š¥å÷?'¤ü4Ÿ¯?èb÷ãÅ.?ÏÊ?'Ñ?Ît#ÀpëG?ÏÊ?'Ñ?ïoª%
¯?'0÷Øáz?'
»bº6?'0÷Øáz?èXÐãÕw?´
Fáko?Μ¼p«†#?´
FákoAGN4FGL J1904.1+3627¿ÏÍÊZ¤Ô@*¾°1‹"GÀ9ê7iDÀ<4†6††@ ÔW§†Â'?üdÓSϊí?µÒ
_š~?±õoÙ+ÕÇ?û£¥Üû(@³†;B÷!?î[?î¿ìêg‡?âú°4撿Ûsµ"[ÄÍ¿Ûk:v"¿âQ¼‹6)ˆAGNbll3FGL J1904.5+3627MG2 J190411+3627?ïþ¿èQ§V?#k§uÃ?$zá$³¨?#k§uÃ?ïìE¤°?jꔤ~?cº\6©‹²?jꔤ~?ïøƒ€ÂL?E?vHá­?Mñý`êE.?E?vHá­?ïíÌ]ü©?L$ÜÜÇ/d?b3¢À›þY?L$ÜÜÇ/d?ïýû9Wö?'/î¸x?0&3ø£‹?'/î¸x?ï'#`­>è?š{$qK@?‹w'ÍÑ
?š{$qK@?ïõÊ$%ú?b'sƲg­?Tk·Oðå?b'sƲg­?ïå ªSs?\K-õ4‹ª?j_ëTLµr?\K-õ4‹ªAGN4FGL J1906.7+5419¿ïõë[¥(@3œ¯¢ðZqÀ;"§z¡‡À<Ò.d—YM@×3ÞLQ?þy™aܔ?Ðý'üft?à'`ç÷K@M;å‰\5@ºÂá¼s
¿äžðP_"ä¿áûR'L¿Ö#º"ˬ;¿áÁI̽¿ïÿÿ)@k*?Ì=Å]l¡AGNbcuTXS 1905+542?ïd91ò7ã?¢d[öÖŸ?"xÙȘ;Ÿ?¢d[öÖŸ?ïhÇÜü@?š…-$¢ã?'çw?û?š…-$¢ã?ìÓ®K`S?¢ô릌J?¹b£Hg?¢ô릌J?îüv¾MX#?'$uQ"í? 8"ºáÝ?'$uQ"í?í⤆ÌQA?´Ѐ)"Ê?°êÛÊçPy?´Ѐ)"Ê?è¹"ÅkžM?ÍÎʱr0þ?ÍtêQ†Ê?ÍÎʱr0þ?æ]R$©ÇS?¹"ýu«
­?ÓE[¶¬qZ?¹"ýu«
­?銞±}ÞJ?°i³¹žv?ÉՅ:†Ú?°i³¹žvAGN4FGL J1907.2+0126¿º+T­–|ÀãªÿójÆÀ9Ûe˜áöÀ;r^‡tÔ@ lû™¾Øm@WhY…­T?Àè%ü¾Ø?ìá~à†?цW2üÂ@ uT•Ùq?ïÆÏ\Êr¿ê0¿»lR¿ÛåÞs=d¿äC¸§Ò¿ê¡É´˜c?¨y?ÜäÇëAGNbcu2MASS J19071198+0127091?ïñÁø¼ ?WÞÒ¹@íø?\|9»ò?WÞÒ¹@íø?ï¹L½Gô‹?Ì,üÅú?¬Ð®²É)?Ì,üÅú?ï‹æÀ5\%?†Õ?Pç'æ?Oùˆ.È?†Õ?Pç'æ?ï܉ì†B?ZF}"dz?q»	Õ¢°?ZF}"dz?ï]º2ôÓ?"ú;ŽÚ‡?"\(´yû·?"ú;ŽÚ‡?îU…†­Œ?»P-œè¦?ª§®§•';?»P-œè¦?î«}"÷%?œÂÎ>5?¥H&Ë ñµ?œÂÎ>5?ïy"¹›ö?}ä0yÓ¦?Û¨É I?}ä0yÓ¦AGN4FGL J1907.7-1232¿©dtêOÎüÀ"'ãâ"À:|Á>úÓÀ;Ç0ÄÃéÏ@róÜ[50@e*ýÌ=?ÌBÀÄÖ´?°Ïѹñ}Ü?坸ýâïN@4"û§Öž¿ïþ{€©Þ‹?ïø¼©¹L¿èŽÚù¶9ã¿ãlžä²¿å¼ôýîWâ¿äo åRÖAGNbcuNVSS J190748-123221?ïõOiìû
?X2{m€¬N?Ua,#J6?X2{m€¬N?ïZâúŒ?9«"»/ä?4£ ®Œ?9«"»/ä?ïšzØ8eÍ?'mÊ3A'K?‰aIõV(¸?'mÊ3A'K?ïÊ㣨ç?aå'ºjn?zŽ.C™¹£?aå'ºjn?ïÑS€õL¸?vÐɟYk¾?wV?|j¨K?vÐɟYk¾?í')BL3h?¾î]Z	?¶ÆµîzK¿?¾î]Z	?îQ~"Igl? oÍÝðy?ªè½ý>>? oÍÝðy?î#ÏW@¯?ž÷sUº?­ÏƒY?ž÷sUºAGN4FGL J1909.5+3511¿ê:MEzð@'µI@»±òÀ;s•ûg¿À<«a«Ã@"•M.²?üzi¾	»k?Ðmµe'!,?²uÄ'aÿ?åP¾ÉÔÊÈ@óß+ôûj¿êwÄ?ì"Ô}›6¿½Mߢú¿°£ýöjœ¿èžHUh?ÐV±Ý³$AGNbcuTXS 1907+350?ïÿ1¼R?#¢dQ2Æ?¹Á³»B/?#¢dQ2Æ?ïêxN›C"?pˆ4GRu~?e‡±rzÝ?pˆ4GRu~?ïáÿIªK¡?wsÚàdBð?n¶hò.É?wsÚàdBð?ïô^HƲ?C)_n™º?WCÛf3‹×?C)_n™º?ïý;-
æ?3Kõº7?3†%]õU?3Kõº7?ï}½‰Ò–?žYLI? §Ú.r?žYLI?ï·MY	©?‡ÙÚY?',¹ö̲?‡ÙÚY?ïÛOþ+OË?gÍ­ÆŽ?rXÔZš‰?gÍ­ÆŽAGN4FGL J1909.7-2140¿ìû%£†5À+BªŸ{À:1"qê('À<O σ`@O'`Âãj@@×¾˜V£?ÄÏr™z?º=‹ÀÔ›?ôîÊ2¾™-@Àö†""ù¿ïÿæ4|ßO?ïÿ=ba(¿ä¼N/7ûð¿äŒ–ç7²¿ÜM Å¿ïÿwåëoAGNbcuTXS 1906-217?ïòk™ù]F?^o8I)?[(̀¸Sn?^o8I)?ïÃîŏ?ƒˆfVÑ<?~@µ"|i?ƒˆfVÑ<?ï™J°Â?ˆá4ÄÊù"?‰­SÌ
#'?ˆá4ÄÊù"?ïÕˆ`>ã?[qSÝ&Q?ut»Î€¶´?[qSÝ&Q?ïÞÝ;ëú¡?m
˜u&z˜?p'bs‹µ?m
˜u&z˜?î Drd?·!)$Ï]Å?®¥ûº'"ú?·!)$Ï]Å?îÞR¿
ƒ?š÷o™³c?¢ßÁ{rÙ?š÷o™³c?îû½nF@?á	"]ÿ,? O'cÎ?á	"]ÿ,AGN4FGL J1910.0-2453?îžèÜU‰}À-Ø$xGÀ:Š'Úb·…À<+¼•G$'@Zx¥-K"@sf³"@?Í¡¢§ŠH?ÐÂ÷+c±@€Xeã‹@©‡‰Ìœü?íÏ~x¿äò]®î?«ªÞU؜¿éRKý."h¿î±†Àyt¿á"Év7AGNbcuPMN J1910-2448?ï¸<t¥nd?€oò:l?ðâÖLpþ?€oò:l?ï©{Ù¶¯?'zÆ?…¡'³N?'zÆ?î¡Ò9b/?–¤
¤/?¥âÜi
?–¤
¤/?ï!ƒØè?€{3q®Xl?›Ï"ܐ?€{3q®Xl?îýAKq9ö?œC,å>? +ëHì`™?œC,å>?í«ÓõØV:?ºÖ˜=#!?²¡`Q«A­?ºÖ˜=#!?ìB=kM½?¦Òk43?½îl¥'?¦Òk43?ìONÝ?£Ñ».uÑl?»õ‡M‰8?£Ñ».uÑlAGN4FGL J1911.2-2006¿Ø­PôAäZÀ*v±=û
RÀ7΋8§À;<18‡0@}ædÌ@×Å>c?ž_ßÛê™^?ŦZݜ'é@$±Ë«d9@´œïd|V¿Ì8Lw§×J¿áÎÕ»ˆ×ª¿æ<tZDïô¿ç{tëdg‰¿êÿ`Ónu¿ïþê šª;AGNfsrq3FGL J1911.2-2006PKS B1908-201?ï-ÅÌ/G?¯¦s:Âñ?šGF"
?¯¦s:Âñ?ì6¼L?ÄÇ¿‹Š|?¿JŸ<
?ÄÇ¿‹Š|?í²XÓ^iö?¥ò³¤"WÅ?²m9eè—M?¥ò³¤"WÅ?ï,MÛ*3?"×ÙYóÈV?š}ÖM1¿ž?"×ÙYóÈV?íÔ¯™$¦?¬~…¬UH?±Zƒ7»)Î?¬~…¬UH?ÙÙíÚìþ¤?ÓQbM§þŒ?ã	‰€®?ÓQbM§þŒ?ëÔXÚ©¯?¯›J¬s&?À®ŸÐ•YC?¯›J¬s&?å£ü1qð'?ÀùE"L3?Ô¸Þ?ÀùE"L3MIXED4FGL J1911.4-1908?à(P0NZÀ)Ä£çÑ5À9²×'2tÇÀ<"†4b@ ÁÀÓg?ýªbªCž?¶ã´3gÈ?¢îbÁýL?î,ný@	-ÆJ|¦¿îÝ2K¬§?ïÕdž½Ê¿Þ¶BFÌm+¿ÚNï;â"D¿Ù˜j¥:a¦¿ß'%¡ûAGNbll3FGL J1911.4-1908PMN J1911-1908?ïþ¨·Dh?‹ÏŸ¤åE?%tŒÕ÷ÿè?‹ÏŸ¤åE?ïÜRmNü¬?{øHµïš?qÖÉIcb?{øHµïš?ïëõÁ…p?e)Ew4?d
>³G'J?e)Ew4?ïó¤-'€_?Cx¯²ÁN?X·¤Äƒ?Cx¯²ÁN?ïü9X³˜?1¨#Øڎ?;4VÉð?1¨#Øڎ?î˦®Cäu?³åöCD¡?£E•	ê°?³åöCD¡?ïã3"'K?u‰¬N¹Í?lÌÞ"Ù?u‰¬N¹Í?ïà"¹­$?bY5o^%?o€ÝUq#Á?bY5o^%AGN4FGL J1911.5+0311?íÔ[Gµ‡rÀ-<ÿdύÀ:¨ÕâDiÀ<"y™I@!–YÉË?þ,\\×q?эM{2ü,?ÜÄÑ¢@
Ö0'?ûóHàn•¿çzá³
Þæ¿ïÿØÝý Ó?ïýÖ$dcW¿Òç*{Ԍµ¿Ùi>›A:¿ïŽÎd|[AGNbcu3FGL J1911.7+03072MASS J19113134+0311093?îۖ$6?ôÓ^Gš?®²FŸÝ¼š?ôÓ^Gš?åèbfÉÚ÷?Ð-Û¬èŠ?Ô/;2lJ?Ð-Û¬èŠ?íÙ'%Þ¶Ú? µB[õ=?±6ÆÒT#­? µB[õ=?ë'dÑ2Y'?©FVRQnx?Áöl»6™¼?©FVRQnx?îc%¿,P@?ª?8=øÍË?©Í¤
:ûÿ?ª?8=øÍË?ÓÌpö&&I?ÑBxïï«c?æDŽììÛ?ÑBxïï«c?ë'}feÃ1?®ƒ$	»
ß?Á¶
fhó<?®ƒ$	»
ß?Ýøâ˜ä?ÄO UBl?Ꮃóž.?ÄO UBlMIXED4FGL J1912.0+1612?ê–¥F9å@¿2/'À9ê#'¬?À;3³ÍêÚ@Ùà†"@u±ã<zÛ?Òl¸þæ?ÄÕÄÞõ?ñ'þKÊÙ®@<~€¹xÝ?ÒåÇ5樂ë¿ãåî¿â{G¿1X¾¿ärà цƿè‹6"çƒ1¿è	㮐¡£AGNbcu2FGL J1912.0+1609IVS B1909+161?ïãÄ¢¾Ñ? /Mû'?l;^f¿? /Mû'?﫚Ûì'þ?™²'f²?…H÷ Љ?™²'f²?ï˜ô|$yî?†2M~9Ì?‰ÂàúQ v?†2M~9Ì?ï÷FúÕ¦?4f¼ŽxÔ?Qr
»›#>?4f¼ŽxÔ?ïîºª­µ?Šrþ™^Ä?ˆ"QXÄ.œ?Šrþ™^Ä?íÐõÎL)?»½€‹x)?±xQ›'8?»½€‹x)?í2ӁÇÀÉ?¨}àœ±?¶icóç»2?¨}àœ±?ïÕtuÀ?cÛ1+SU?uEÅ6¡kç?cÛ1+SUAGN4FGL J1912.1-0803¿ï@T.‰À zµ^ñýßÀ8¬™p~îÀ;~^sRÞ@ƹ†sø@"òü~¹?­‰w¸sN?¯wûd9æV?ÿ–xbm@ËN¢$'–?ï.rýMž¿à$åýö:"¿ä—‹')»e¿ã½/
/¿è1ÞõCd¿å',)S¶`AGNbcu3FGL J1912.0-0804PMN J1912-0804?ïýú#È??#8'x"r´?0.á-9i?#8'x"r´?ïÉ*=Á+¯?‡Ò¶°P¡J?{já/èH|?‡Ò¶°P¡J?ïÒÐñ*?~ÌlUæ¶?v—õ‰•N¶?~ÌlUæ¶?ïõ·
Sý?D&ÈqîaÌ?T'ëª|xž?D&ÈqîaÌ?ïøo'Cšñ?Hàð¨vl{?NA»·}¼Ž?Hàð¨vl{?îIÿru­?»ÆÐĈl?«`lZ+?»ÆÐĈl?ï‹Q§^ö}?Œu*
?ª?+–6в?Œu*
?ª?ïè²'H4?^ÓYñé?gM叴?^ÓYñéAGN4FGL J1912.4-1222?âuš
)U±À$n9'ÈÅÀ9PŒAÀ;M¤Ú?|@'ñb~Š@®³Ý¾?¸×4ÀãÓ?ÌÎü|è³Þ@]žvx,@à'i¤‰b?찔[p¿×"¼uf´j¿ã"Àíp†¿çs¢¡¿çG8¤¿ïÿôA…ÜMAGNbcu3FGL J1912.6-1223TXS 1909-124?ï9QlŠÝ?œ—›(?˜Õ߉מ|?œ—›(?îِ'Õwc?§¡Rm­w?¢föä`WÓ?§¡Rm­w?îÎ…oÒ1?™Ei«:6û?¦ó«–'ê?™Ei«:6û?ï>Õfµ|à?€>ØX Bê?˜%S,¿ÿô?€>ØX Bê?ìpŸšÒ?¸â'_REÔ?¼{+ƒ'o?¸â'_REÔ?é𕞄²N?ǑàóÊ4?È=©…í6Ç?ǑàóÊ4?è'%D"|?³&j™5"?Í·kÞí®?³&j™5"?éÄϬG"?°Ê>ôç°ï?Èï˜ÁNá²?°Ê>ôç°ïAGN4FGL J1912.4+3738?ïÿûìR¬©@(´¡ß¹8›À:š.$ÖyÀ<CLu#˜‹@›C×ñ1@LG䛬?Å´'åLJ†?·Þh«?ûU_]]©)?ÿ|Øm¿Ì?ïîõ üпâcåîy¿éûP£†'f¿ÞáÉÿ={¿ïÿ~›'?ïõ!¬ˆŠAGNfsrqTXS 1910+375?ïϧâmÚ?z8zÄ!?xr,(6.Ø?z8zÄ!?ïb"îM]? v9i?"¯b4¦Æk? v9i?ï¦áHYàò?~øàò3¼®?†G­ÛÉS–?~øàò3¼®?ïLí"¤Œ?z¦y(hÝ?–bM}ns?z¦y(hÝ?ëkí7?K?ÀEÂw<?ÂQÀK#Ó?ÀEÂw<?è݅6‹,n?ÊË6ErŒ ?̉ë%ÓNF?ÊË6ErŒ ?î}ÜzGwk?‡¿64?¨"8]@WF?‡¿64?èÄâ<ö€z?²³P›?Ììw%þ?²³P›AGN4FGL J1912.7-1250?˓vñ4FjÀ$ú#9ÀëîÀ:&êÏS)À;ÑÛ¤$é@ 
¿)öôi@BZƒU?ľªŠ­˜?±5ä¾[?ðãœ*Ù@oL¶çÞ ¿ïæó{??ïzOßK¿ådÂÝ_¿áà³~È¿äxgêŒÑ¿è…2ˆKAGNbcu1RXS J191251.7-124929?ïûèD³Ÿ?;¥XŠ'?C˜_Sr®©?;¥XŠ'?ﶛïy?ˆ¢†•?s²?'x>&j›ª?ˆ¢†•?s²?ïà
ŽUe/?rÚj?oòq¦{I`?rÚj?ïԘAĊM?\äÑÓ·?u³ß0H½t?\äÑÓ·?ïéXc'?g¥3æjb^?fo§ÌšõP?g¥3æjb^?î‹ëÛ?±mÃÍ«·?§AG0ÐP?±mÃÍ«·?ïlji€LA?'ƒ]ê?'r²ÊÏ
ó?'ƒ]ê?ïżžg›?'!NŽ–KÕ?žgHtÊ™?'!NŽ–KÕAGN4FGL J1913.0-8009?ïŸX1ªÀ;žêúµ=dÀ8ãÜEԉÀ;·%;ù«R@yiÓ®=k@±ƒÞFqÔ?«Îªžœ8?ÂWzzÅn	@§Òª\_@:Ë-?€{¶@ˆ¿ßÓ þ½¶¿åìÉ⌧™¿æáìï'{¿ê{÷"J¿ïÿrÁ¾{ÑAGNfsrq3FGL J1912.9-8008PKS 1903-80?ï÷`ɐϓ?I…´lE»?Q>l†jږ?I…´lE»?ïó±‡IF?b-"Üiì?Xï"çÓe?b-"Üiì?ïÉÕ­à½3?ræXcÂ:Ù?{)$îú-?ræXcÂ:Ù?ïþKÂB§'?y¢5ZÑ?+Cܛpb)?y¢5ZÑ?ïë/.Òâw?^‹S!"'?dÐÑ$ÞyM?^‹S!"'?ï×@ø)>?€VeuyL?t_ƒÓq?€VeuyL?ïZ‡	
Á?'pàŽ¼?"¯ã†QÝ?'pàŽ¼?ïùNlìß´?>-/;Þ?JÆKÅЀ?>-/;ÞAGN4FGL J1913.2+0512¿æ™5‰W_ÁÀÊ›š$ÚÀ98
¢pÀ:ÕÈ­ç.@ÀŒL©ý@úo?Rü&?Êj»ìÕ¬?Ë­G`ç¡d@¥s!_Ì@KÿßÝ6?ïJ|€Y+À¿áU)' ¿éøn¦¦ÈV¿æ¼o»¿êě¥ãSø¿ïÿI)>¾AGNbcuTXS 1910+052?ëמ
}Ë?Àôè}`?À¡‡ÖñÒ?Àôè}`?çE¹mÆ?Ç$†5þXz?Ñu֍ã$t?Ç$†5þXz?éèRKž±S?±ž½6ÃÔ?È^¶Ñ…:´?±ž½6ÃÔ?êûÔӒŸæ?ÑïËHc?Ĭ±µ€f?ÑïËHc?Öf&1f‡?Íêýàý¨?äÌìç8L¼?Íêýàý¨?ÉêiËu´¸?ÍNå(ÁÈÀ?é…e"'Ò?ÍNå(ÁÈÀ?Û[X×ò?¹ê= õX‡?âRS"&ÿ?¹ê= õX‡?ÏøA–^Œä?¯Äìõàb?èïšh\Ç?¯ÄìõàbMIXED4FGL J1913.4-3629?Ôðýsˆ¸ÌÀ3ÚªŸ{ZêÀ9³æ鮄ãÀ;'ŸJ³'@ë€nÐBM@$FE^¯?»ßð¯š?ÅÀüI'I@ˆ=ÿ?à@4¥/úĂ?Ѫƒ ÜD¿ä"²ªØ¿Ødñ†Ày¿ä'Ù‹÷ð¿èÈòýãñ¿êy
By!TAGNbcu3FGL J1913.5-3631PMN J1913-3630?ïŸ{W(Ç?¯4udœfò?ˆ!*9gêE?¯4udœfò?ïȝxKk8?…¨aÙ¸
?{±CÞiëÌ?…¨aÙ¸
?îÒ©ÂJ?—ò·pBU?¢Õcߣi&?—ò·pBU?ïÚWæàŽ?[|x€Ø1?rÔ{PÕ?[|x€Ø1?îë÷¯v?¦+d‡¾û©?¡@ŽˆÀï¤?¦+d‡¾û©?îÀsð_?ºéƓÞÖ?¯ãø¼®‹]?ºéƓÞÖ?ìFAáTw?ªŸ*Cž°ó?¿Íðõ\I?ªŸ*Cž°ó?îëþ­Ö¤?š]¡·Cz?¡O ²ùË?š]¡·CzAGN4FGL J1913.9+4439?í;´î×,@-ó*k
•À:I¤¿g‰|À<t'Ç=@Ó@£%2g±?ÿJ£ý ª/?ºK_ú¼t?©æª!.×b?ðs
=Ö$@*fÅû?ïö Kºi¿éï=n¿ÒeÎÜŸC¿Ù÷½j.G¿ãV½¢…¿çT‰Y°u~AGNbll3FGL J1913.9+44412MASS J19140184+4438323?ïüùÔd=?1_T"Ë$??`0ÿh¶¼?1_T"Ë$?ïíƒÃjò?dºGzm"{?b|<¶œŽ0?dºGzm"{?ïõBé[?c4.ì3½Å?U{èQ9X?c4.ì3½Å?ïϦª_uÃ?\
Ë@?x,ªÃæ†Ì?\
Ë@?ï÷ØÙöV?L¼ÙŽ6?PNLH¼E?L¼ÙŽ6?ï¡á¡1¥?"žºOM™\?‡‡¸årÄ?"žºOM™\?ïñÑßӇ?pÆ<?]Ê\Y!£?pÆ<?ï€['‡c?vOW×Yz?øé
pq?vOW×YzAGN4FGL J1915.3+1149¿âïáÙ?ö}*"=mÀ8vW0h}˜À:º|h0@љÅäPL@k9ýQÏÖ?Ã`qšL
?ÖFíD'o@¸0]•Ý@™Õ­œ¿ÔµŸ^ª…O?éO/]e¶¾¿æ	!ay—œ¿èy‰Ž‰›¿ïþ›{ñèæ¿ã¥ÁX¨8AGNbcuTXS 1913+115?¬H»X ̀?¾'Ûš£l?î;tJT·è?¾'Ûš£l?¨ÛZš…pÐ?­~kH?îrJV ¯3?­~kH?˵ëx£?²îÞÅð%?é9~R…!×?²îÞÅð%?ºÇóxvøõ?¡mép$2î?짐ñ á?¡mép$2î?lU3¹	ý?t`Óä?ïãªÌiG?t`Óä?x† :?†]âõˆKÌ?ïÏÂò/À?†]âõˆKÌ?¥ðÖ=ûy?š‡Õ"»ÿ'?î ò›éU?š‡Õ"»ÿ'?`˜%'D?TÀ=;¯Œ€?ïïgÛͳ?TÀ=;¯Œ€PSR4FGL J1916.7-1516¿ï÷ØÒû¡2À(Èõ\)À9ÌѝìåqÀ;ÄSõJšX@#>¥ØW@oúcÞÍ?Ãû×ý,'?Ðô!ºåĕ@ð@|ÇÑ»@D]ÓG?ï¶A……¿áøŽâ[X¿éƒ†="	¿èTÒõ۹пë¨"HK¿ïû÷"IôAGNbcuPMN J1916-1519?.ø!K?¨o€À˜"?[´>ˆa?¨o€À˜"?ïÈRzSá²?'º"g<[ò?{ÖÂåÝZà?'º"g<[ò?ïøà?'ÔµkµšQ?ž`ÿ»Ëþ?'ÔµkµšQ?ïáÈætyá?SÈä`îR?n7Ãß·
?SÈä`îR?ï]%cւó?"îY¦/A?"[S€7­?"îY¦/A?î"ÈÍÊßÉ?±$$(êŠ?¦³s ¾Nu?±$$(êŠ?ì‹ï8Ú£?§,Ú9Øúê?» †?A*å?§,Ú9Øúê?ïJ'…·Ô?`‹úm¯?–»f±ÿ†?`‹úm¯AGN4FGL J1917.7-6442¿"•/®l°À;•»¾‡À;	ÏDvQ–À<ªJaÎ@÷\"ë'`@œ2?Ñãâ» ¨?ÕP–ñH­@=p£×
=@'ŽÇ®Û¿ïÿÇ*Ì\e?ïþΈ°=¿á%Óύd¿çòùℚ¿ßë,~Ž%r¿ï¿ü¥¬¨AGNbcuPMN J1917-6435?ï÷$Î?O®·1àÅÏ?Q·òšó©?O®·1àÅÏ?ïêìŽoU4?jdëíosÇ?eq–*,Y?jdëíosÇ?ïrh©ˆq?ˆW╆?'²þ1®)È?ˆW╆?ïç²%5]?QôáGéÞ?hMí—rJê?QôáGéÞ?ïóf17ZŠ?U…q(Â-?Y3ÙL;?U…q(Â-?Aܐ²?•u¥.ßL½?‡ï…l7¢?•u¥.ßL½?ï`¦LÊ"?"¼§5šˆÛ?Ÿ3ë/‡ƒÍ?"¼§5šˆÛ?ïZrˆ™Ó7?‡dëé§áÌ?"±®ð55+?‡dëé§áÌAGN4FGL J1917.7-1921?ê.Ü2µ"ÑÀ,¥(IË%-À7õ"i†¬WÀ;jUõÕÛ@âÈހ©^?þšÈ:£j?šlûÅ¢zØ?˜\ÄÙ?üp'|F¢@:ŒÁnö?à­ÆÂqª¿Ò‰½#ã4¿à_Ðéſ۞üd¿ó ¿á5Мe&¿×èÔjOÿóAGNbll3FGL J1917.7-19211H 1914-194?ïþT3*q:?Y´ÛñN?*¼Ë£QS}?Y´ÛñN?ïÕó®l?|.Á2á'?upQÞ9?|.Á2á'?瀞*yŒo?‹"/ˆ;?…Y5o[T%?‹"/ˆ;?ïëÜÔE«Ë?W¶Þ/¿?d#+㏅9?W¶Þ/¿?ïùøŠHK?B©Œ…cÛ?H™6ä6"?B©Œ…cÛ?ïBtø-+?©[k]1ŽŒ?Ÿ7±[Òð›?©[k]1ŽŒ?ï°ûϳuÓ?Š4S…lø?ƒÁ{Án?Š4S…lø?ïá®ÐQUw?laõp¶?nQ/vPñ`?laõp¶AGN4FGL J1917.7-6930?è ²ÕªÁàÀ;' hUSïÀ:NãF¶žÀ<p(ßó@Òë1¼»ˆ@SX"?½qõ:Õ?'Ç]~4Ê?Ô$ þè¨Ë@
0#	ÅP­?¡UMºHä¿ÛIÞ}¿äzï,D¿æ8}¿H€¿ãÈM Å¿Ñ×DÔñ4AGNbcuPMN J1916-6928?ïÕ¾BÆN.?®Ô">ÜjÂ?u ޖ©C?®Ô">ÜjÂ?ïöWf³8?Y_¸Yp²6?SQ2Ó¶þ´?Y_¸Yp²6?ïñNŒÞ}Ø?eKŽX¦À?]bæ|½À?eKŽX¦À?ïÿV©ÒCQ?TìÀñÈ0?*É (t¿?TìÀñÈ0?ïýŠÉy?,"tÄ:p^?3©¹†U˜5?,"tÄ:p^?ïÕ©@iÁ?"?îjÙW?u+zXëç`?"?îjÙW?ïðƤó ?h"g
1¦{?^r¶ˆïv?h"g
1¦{?ïþ9!ÅÞ­? §¾›"Å?,mæÉÏ? §¾›"ÅAGN4FGL J1918.1+3752?艊^N{@&à=ݱ ŸÀ:Â7n+VÆÀ<vÒõÛ¹Ð@ |ú<ü¶?þÓCßRáN?Åb}äzC?¿H‡h:&?ùf'•ù@sBdÔjü?ïùfˆË?ï³!å#¿Ð_¾+Ÿ@¿Ý0¥dSÉ¿äD-÷Š¹¿ÝfN=¥§ðAGNbcu3FGL J1918.0+37501RXS J191810.2+375315?ïþ²íù:?7¯tÏ?$Þ.ç<Ø?7¯tÏ?ïÞÁŠŠ™2?y'(øKõ…?pŸ:ÒÀªö?y'(øKõ…?ïõüÍVƜ?Dà«óLÚB?TeÀfF?Dà«óLÚB?ïÏFåìG?^®°__]G?x\ü S?^®°__]G?ïû¾e3"
?<½È~ºr?AkúYè?<½È~ºr?ïEáÉ^-]?¢—‰g%Ò?—CÆÙa¾^?¢—‰g%Ò?ïï©Î'Ç?kbÁ©¿/?`V1Ùϑ9?kbÁ©¿/?ïx:1è?'zѹbæ?ø¿™Þb÷?'zѹbæAGN4FGL J1918.2-4111?Ê£üóAgÀ6=cEI¶,À8^&åGÀ;wF'‹ˆ_@3,éŠ?üíy¾Ô?¢ð"½DC§?»œÝø©Ê@ãÔHµ{@ó8–õOx?±
9>æ¿Ø6êx´G¿Ú
Jk^ì¿ÙÖØ9¦ë¿äw^o¿ç;C£AGNbll3FGL J1918.2-4110PMN J1918-4111?ïõ¦.l=Û?{6žù"Í?T³¢žë‰?{6žù"Í?ïÄö†ô??…Üåb‰¦Ì?}ø°'Hn?…Üåb‰¦Ì?ïD6øS}?•æÃÇT7Ç?—y õ\Ñ?•æÃÇT7Ç?ïÀNѳð?fXGW#?ØüˆÀ#?fXGW#?ïÞôKZ¶?xƝKåè?p…Ú5MB?xƝKåè?î՚ÄÅtò?´sÁRg?¢¦S³¨°Û?´sÁRg?ï{8¢ïë?'<%§×´?¸äÂʱ?'<%§×´?>‹oÏ?"ê›U5°t?§×m?"ê›U5°tAGN4FGL J1919.2+0618¿ä)ÞTC#À
!ÇÃx5À9wEšMôÀ:ö@&t@õøADÃÔ@ïOP ?Ù*æÞpä?ߋ:[E ô@	áZùJÚ@ÉIýúí¿Øí‡Â׀…¿àâeàÚuØ¿ê"¦žô:¿ïÿÚv»œ?ïøÍaO—¿Ï€™XG#AGNbcuLQAC 289+006?îSy=^?¾ª"Dë?¨
ÈkJC?¾ª"Dë?îX$¦Ÿß?ºJMÛC÷À?®*}³Þ4?ºJMÛC÷À?é×>\Ôc¼?±*:*z%V?È£Œ®q?±*:*z%V?ïó^OSÜ?VÛ»aôFx?YCaZä)A?VÛ»aôFx?ç†HÈ,d?Î/7
êÒ?Ðóno§á9?Î/7
êÒ?ÚUH$°¦?Õ_Yí1FI?âÕ[íø§­?Õ_Yí1FI?âœÀ"¢õÁ?¸ø¯¦6»?Úƺº}?¸ø¯¦6»?íSO˜ø¨?·'i¢ò8?µeƒ9‰MA?·'i¢ò8MIXED4FGL J1921.3-1231?ï«ãÎq»À(|Ä&5ïÀ9þ‹‹¹ÝÀ;ÙQAK$@ìÀÜ©Ž¯@$'ÇÅ&?°€m"Ã#?°ö AÏ@0
ø'@ªÅÎÖ½?çÏó"
3`¿Ðÿˆá»q[¿âA:û¿Þžœ)¥ì¿á¿ï~Óo©¿äҌ)nŽSAGNbll3FGL J1921.2-1232TXS 1918-126?ïø§p3?CÓ® >:?Mc†Í©wì?CÓ® >:?ï ๋?oæk$(c?‡úGÀo,š?oæk$(c?ïé.å5Y?g‹OZ'kÎ?fÑÒMÇ?g‹OZ'kÎ?ïN©½yý?~Í""ËŹ?–*ÈZÁ$u?~Í""ËŹ?ïØPuR+`?olŸ¶¢<£?s×Å?Œø>?olŸ¶¢<£?î.»–æÙ5?µæ@y ]Œ?­F¶…³?µæ@y ]Œ?ï´-9§Ÿ?†"+woP¯?'ÿ4·mn0?†"+woP¯?í|²Ï[ف?œöóÜÊ?´iƒieü?œöóÜÊAGN4FGL J1921.7+5817?¦,XnC9@3	‡¤¤—À;Ãú%Ëk¤À<õçoæAé@!×Û[/ür?ú}$ƒmj?ÐÃqnØ$ð?¼Óæ``º?ñ§Sçáv@öh@†-?ïÿÍ?¹Ss¿ïÿ'ÌÎzL?ïÿ°ï÷t@¿æ#Ã>-¸¿¹øk µW:¿áG»ëÓùAGNbcuWISEA J192158.68+581708.5?ïþ}ùôÝ?öYÇf¾?( o¢\6?öYÇf¾?ïïÌùîC?b«rýÖ?`3Þâ´ ?b«rýÖ?ïçÿJÎZl?h³6€Ÿž?hµjD³?h³6€Ÿž?ïê†;mê>?Q÷äÄ"¾?eyÄqá?Q÷äÄ"¾?ïþ]9c?,Ñ¥Q!±?*/<w•?,Ñ¥Q!±?ï¯}N½ÛÌ?Œo¹^_?" ¬A»"?Œo¹^_?ïæ©&vٞ?räsC+ìH?iVÙÆÿZ?räsC+ìH?ïÇúNvl?t䢴l!?|uÍ'?t䢴l!AGN4FGL J1921.8-1607¿îšŸÅúíêÀ+¾¯«SÖAÀ9NjXŠÜÀ;¹ðál—@ )`^dL?û;=Žc?²c/¾ù>_?·m?Énžn@Ѭ€&+
@
ïß´tç?6ä•¿£Ó=@§¿ØÕD€ª³¿Ð*b{ö¿áa'Ú¿×IÅEïÎZAGNbll3FGL J1921.9-1607PMN J1921-1607?ïý¶´)	[?(ÃæÇÍؤ?2J`ÜW?(ÃæÇÍؤ?ïÂ(ˆ×¡ß?Šô63G?~뻑o`V?Šô63G?ïÚ¿ŽBDë?u8"Üî5?r 8öêÎ-?u8"Üî5?ïçlȟì?N3ŒÕÍ/ù?h"ð7`'?N3ŒÕÍ/ù?ïúxà8i?A*Ó¦c?Fß֌6?A*Ó¦c?îµþK
ß+?³>fB?¤ OýôV?³>fB?ïÆú o¡£?ƒû—¼Òà?|'¯¬²Ng?ƒû—¼Òà?ïÇٝby?j&[ęœ?|1]_Ÿ?j&[ęœAGN4FGL J1922.2+2314?ì2~ZŠ @!0¾
í)À9Ò°@¥¾À;¶_ !¸@ ˆaV݁@x˜:	?Â^´Á=L'?½Zž\! ?ýEª~Ä+>@âw¯äà¿ï²xË'u?ïüá½tÀ¿á8&êþ¿ÛT÷=¹žó¿æUF˜¶›¿àjëø?AGNbcu3FGL J1922.2+2313MG2 J192213+2317?ï÷‡dҁ[?P¥×R}I"?Pñ5úÈ9"?P¥×R}I"?ïj2=úÉ? S»-±÷±?'¹¼Ñanö? S»-±÷±?ïÕܨ?û?z¢«ºì[?uüJÌ~Š?z¢«ºì[?ïpþ
b?vÄ1'ã?'ÿ…e½Ç?vÄ1'ã?ïÎÑÅì*?uwt&§?x—þD¿O?uwt&§?ì‹,'˜Ì?ÁÚšã+?»¦žÇ£9£?ÁÚšã+?ï8DŒnZ?™w´Wæö?ž˜÷k˜¼?™w´Wæö?ìÌ$➬d?©«zH™Âv?¹žØë
œÞ?©«zH™ÂvAGN4FGL J1922.5-7453?ìoD'ª®"À<#ædM‡À:Õçþ{À<fH;Øô"@ Xr…®€?ýA"d~.Ú?½î^Aÿª?°!a#±`
?ógû&|k‹@	™Ñ;Ü?æ|
A±ü¿ã¶Ã«»Û
¿â2§Ý!ž¿ÐJoD³8¿ãâ"i·S¿¿Õa8¿!œAGNbcu3FGL J1923.2-74521RXS J192244.1-74541?ïÿ.£›??u3NÇ?#?z+¯ÇSÂ?u3NÇ?#?ïö"ƒTU9?Sº´AF¹{?Röù+ZÉ?Sº´AF¹{?ïõÞ?ª©¦?jÑ˗t!¤?TC€ý#SX?jÑ˗t!¤?ïüFùþM?'˜cA9êÏ??ÈdÔcù?'˜cA9êÏ?ïþÓ#¤S?\G‡ã?"ÏÝèê
&?\G‡ã?ïÙ£C€L/?€9ÿ"3K?s.^RgÌ-?€9ÿ"3K?ïüÀ›ø)Ù?@·Â+'?9û åÑj^?@·Â+'?ï÷Jj?A6¼¦‡Ïå?QÁl=ã1à?A6¼¦‡ÏåAGN4FGL J1923.4-2503?çÉ½ßÛÀ1ÄþG™ÅÀ;w/âEÛÀ<£|§‹@"RßÛGcí?Ø©Ý3¢D?ô[D)$¼?ïÖų,é@X> N¿@`̇­ˆå¿æ¿ŽU˜¸É?ï"Fj^¿á/ÿ¢/?ɅsFô†$?Ætð'^"‹¿é0…;=ÄAGNbcu1RXS J192325.9-250228?ïóýJÃóŠ?[³M¿Þ?XjÖ<?[³M¿Þ?ïºÁûk#m?'²­x×?O˜<Å?'²­x×?î©ZÞ·Ÿ®?™Ùòd]K?¥jRõ¡?™Ùòd]K?ï÷câ†%&?Io÷͐V?Q8;ña?Io÷͐V?ïÍXè›×¯?|¬€§\\?yS‹ æ³?|¬€§\\?îU±—&?³Uýs6?ª¤æ‹²À?³Uýs6?îþ[ sN=?—»CòÏê? M÷N:?—»CòÏê?ïòÌϯ?b ÓZhªÜ?Zg÷ëžq?b ÓZhªÜAGN4FGL J1923.5-2104¿¹8PtJ/À0>îؐOnÀ8¡Ïi_?+À;¨''ûÈc@øÄI¦@	<Ú{áù?¥òÀ§Oµ?ÁÒw[¬#4@ù&âÂØW@0—d54?œ!¿Ýø¢¹ì¿ã×Tæb¿ãÓ?ãDÞV¿êüí@àšà¿ê«hÎör¹AGNfsrq3FGL J1923.5-2104TXS 1920-211?ïêåSÐÀ?dʐ¡å?e€ÊkϬ?dʐ¡å?ïÁ½eë[?"ÂßK(Í?v!köÎG?"ÂßK(Í?î¼âcâÓt?™Ñ"»'È?¤1Ù¿?¾?™Ñ"»'È?ïÿTíÔ?™?½'ñ¾Úß?bJB9Ät?½'ñ¾Úß?ï¹'¦¸'?€pC
Ð?¶H]=?€pC
Ð?îö{ƒX?±^õ¡܄?¦ð˜Fì?±^õ¡܄?í¹…ü?t?£?	ïÙ?²3Ðã[_?£?	ïÙ?ïþ"M²îÞ? ôðæçó?&»"ÊòØ? ôðæçóAGN4FGL J1924.2-1549¿ïï"îJÀ,†)Ø@žVÀ:õ™ÊARÀ<EÏ¢j"´@ È¿èbÕb@`b
·'?țëƒq9(?—;ƒ8Ú.?Ó ™?׆@k¨÷/¡Ù?ïµ;K/©;¿ì'Ë $c?ÞQmü÷¿ê7‰Úõ¿œÚ»ç'
¿àõ¶€Z-sAGNbcuTXS 1921-159?ïýDԛMN?4d"mü°?5ÙYuyæV?4d"mü°?ïسÚÚÎå?}p2'§‡A?s¦pìas?}p2'§‡A?ïÛȶ—½?w¥"…ýÀ>?r÷²r'??w¥"…ýÀ>?ï÷âx
`n?>ÁDž ?P;WÌA?>ÁDž ?ïûWÊAW8?BÓ¿üçŠ?B ×°}Ø?BÓ¿üçŠ?ï
A"lU‹?ªZsÔá4?ž·Íuäê˜?ªZsÔá4?ïÈRéÿ/?yí é%f?{֊óYðŠ?yí é%f?ïâ¡z0"?dG(\çHæ?m^玌
?dG(\çHæAGN4FGL J1924.3-5458¿ïáԤÀ:"œT]À;OÖNUÎÀ<Ãü7ôc@ I£ÿyw?äԌê^®?Ú|"zÔ1›?‡ça@9ÞýPù@'²¶v??àbñNŒU¿×AV¨¿ê\vXKñp?ևáá1à¿èâ¬K¿ïþ Eð¥AGNbcuPMN J1924-5457?ïô|¤É×?S$"žßÿÜ?W¶›ÿ?S$"žßÿÜ?ïèœHløž?sÏÈ l?gc·¹ƒœ?sÏÈ l?ïmeÅÆb?…¢¾þðñ?'SG@T…ž?…¢¾þðñ?ïÓð~>¯?d¬‡š1`?vÀÚp¹?d¬‡š1`?ï¹GÓd|½?"d좂ÜÌ?®*Plœ?"d좂ÜÌ?ﶽÀ%°¥?¤y^ %M?'Pî¬¼Ó?¤y^ %M?ï

Êm÷Õ?•'¥`V"Ó?ž^F«aÍb?•'¥`V"Ó?ïÊ[p"Å?xÙuš;v?zÒG«¨Ig?xÙuš;vAGN4FGL J1924.8-2914¿ïâ]íúxÀ3›ûz_A¯À8ªX-¾À;×/¸ToÄ@ú';‡@ò\f2d?¡¯Šœ¦"T? ¤!²Ø/?ø.8øo@‰ê¾ÒŽ¿À–—Ü€¿â‹…Û¿æþA¹Þ³¿ã8î~Mbß¿åÙv0¿ê$-ÁÚ*ƒAGNfsrq3FGL J1924.8-2914PKS B1921-293?ïþ.HŠ)Ü?!/\ìß?-zÄ2gÞ?!/\ìß?ïÞˆì"?€ò.Âö^?pòÿýK?€ò.Âö^?ïÁ[ÓC*?†&þ\ìÞô?RyôJ±?†&þ\ìÞô?ïÿE;Y®ƒ?—Ì=VÑ?X"WÖ1]?—Ì=VÑ?ïüpBՊ?9{€–kô‰?<}êº ÆÝ?9{€–kô‰?ïSˆ_¬Û?¬(ڑFéè?žõŽô
d™?¬(ڑFéè?ï­z>,	?ˆc·8¶·?"¡pqáË?ˆc·8¶·?ïÿ^BØ?s–›k±?t7*º?s–›k±AGN4FGL J1925.0+2815?à-OJ"ÍI@AS½vdÀ9œIlÊ.À;þ)ÊÔ¥@ W)HΦ?ÿW¹Ëh?´øá.-»?¤ý"ãél?òÛHZ⤥@C ,pKm?ïÿ"å­nc¿Î‡ rÑ®´¿äOÉkï<¿ÔrÔ§7¿Üø°WK@¿âÁ6á¾vsAGNbcu3FGL J1924.9+2817NVSS J192502+281542?ïøÀ÷蕑?C,g3B–?Lü Œñ'?C,g3B–?ïÉÒÏp@/?†…ž‡a€?{˜,c¯?†…ž‡a€?ïâœx­L?p)í§³?mc‡†î"?p)í§³?ï­my*8c?i¥‰'<r?"¤¡«#\?i¥‰'<r?ïíBz<ËÒ?`ÕöÑÛ?b½…ˆæ=?`ÕöÑÛ?î̈́Îd??°ÇßÁàÏR?£'³/X?°ÇßÁàÏR?ïÑ×û¡mñ?}Ï©ØúU8?wJûz?}Ï©ØúU8?îäN1=?ˆ01…õ¢?¡»ïK",?ˆ01…õ¢AGN4FGL J1925.1-3358¿¹™›ïužÀ5H¹ý½/¡À:qè«O¥À<‡çÀn@Ôíè¦G'@ԏ¿%D]?Õmfr{?ÒãízÂ=þ@lû%¥«÷@•POù'~¿ÆIà‰B3¿ém2}«§c¿àê^u׿ïü?OQ¿Ï‹Å›€$¿ï©$Q ˆAGNfsrqPKS 1921-341?ïҙ\T@?¯4ÃÅÖÓ%?v³Q׳7ª?¯4ÃÅÖÓ%?ïÙØ"ÁK?}ž2ˆ¥ïÖ?srý
¶e?}ž2ˆ¥ïÖ?î­+ŠzöI?™n3–Ä?¥-GTàÿu?™n3–Ä?ï÷Ï
³‹¢?9ÙñO•?Paä&VF?9ÙñO•?ïù
Á,¹$?WbI Ì?KÔûÇæ?WbI Ì?îh¹fWf³?·¥ÂKBi?©ti›e{Ï?·¥ÂKBi?î'-Í(ùZ?Ÿ'c´=[?­#/(8c?Ÿ'c´=[?ïÂàZWÕ?q¸;{!?~Óáù'?q¸;{!AGN4FGL J1925.1-1019¿åL5³@3ÍÀ(@^_0çÿÀ9"¸:n×À;†¸›½`H@Ì®EM<@Ò<B¦m½?Á†Ë¡(¯!?½lvìÚ^@`GMœk@¯Ôà—"ì¿Ùû/€÷e?ílkûѝ¿Úö` Éd¿ã,'Ž2]J¿æ>o;÷ýÓ¿í0¯_Ô{îAGNbll1FGL J1925.1-1018PMN J1925-1018?ïà¿kmêÈ?oÞ«ŸQ$?o@"}w_?oÞ«ŸQ$?í»l=&7?²Ã££¹?²'Ÿ`¨Ã?²Ã££¹?ïP)^PËÓ?ŽzgÖý?•úÔ7žS?ŽzgÖý?í†j<߯?–Hº÷­ä?·ã̯ÐЃ?–Hº÷­ä?îo@ãȒ?¤~Õ?/	?©ÿ¨å?¤~Õ?/	?ä'1ÖfÔu?Ñdz"¹q?ÖûœS2W?Ñdz"¹q?ì­¿°¦óÂ?­Š#òÝß?º'zÈaó?­Š#òÝß?⠝í n?».Þǘ|Û?Û¾ÅÐ%¿$?».Þǘ|ÛAGN4FGL J1925.7+1227¿æs·8L2ð¿ü†«pÀ9á²7QÀ:È[;ù@¸žÅÓ^a@§;ãÛÝ?¾TÂ(Y?ǸMú3ã1@ïƒæ©í¥@ë9Û׿ÁÙ}µ7"Ò¿á¡Î¡¹"Ì¿ãȑûž¿åªÆÇ©¿ê|=2v¿æÍÉ¡õÔAGNbcu3FGL J1925.7+1228TXS 1923+123?î³Ê«èÚ?±£Öiö?¤ÏR­½a?±£Öiö?ïˆð-òN?š…ÌiAæi?ÃôŠKµð?š…ÌiAæi?ì]£øJÝ|?¬«á+êÄ£?½à=©?¬«á+êÄ£?ïîãÙ6p2?K´rN"'?a&žô¦?K´rN"'?ê꼫†Dí?¿×ˆ½~P=?ÄU
QæìM?¿×ˆ½~P=?ìµ<A³¦?Ã2Ù³²kð?ºV÷jbÓ?Ã2Ù³²kð?è{9¢–¡?±®%°?ÎÓu¥|?±®%°?ï"áñg-?zÁ7" ?ŠÇœyW`¸?zÁ7" AGN4FGL J1925.8-2220¿ìlS€ÁÃÀ1?´åOz'À;GoçïhÀ<ˆÇ:¼"p@"!ëu(?û¦Ô€u?ÎMoÊhC‹?³¹? Só?笇²çHy@'Eã-¿ïö^½|?ï±Oޏ—ã¿à]LÁú‹Í¿Âï,ÉÍ¿â¢y|¿ªYÆ<\I$AGNbllTXS 1922-224?ïþ5èÂg?#6p=ˆ
÷?,¡®ÄH¤?#6p=ˆ
÷?ïÑjüÖ³^?ƒ.<TQ]?wJ¢dÀà?ƒ.<TQ]?ïåÐà"å6?h>¡™Ië?j/¡´±Õ?h>¡™Ië?ïí`)‡?Kᑣ0o?bŸôÚ¹p¹?Kᑣ0o?ïý"¤7,g?/÷GnÜ[%?3bàbxþ#?/÷GnÜ[%?îØö¬<?¬hŠ(ɉ?¢~­% J?¬hŠ(ɉ?ïâB?j¤?uÏ~v2?m½À¹â?uÏ~v2?ï«û¡K"©?{GxN˜+í?…ºÙE±?{GxN˜+íAGN4FGL J1926.1+2059?Þ^ìD®±@v]¤öÄîÀ9†V›HÀ:÷¶‡æê@Ð"—¯Š@ž9ÛT?ǟ¬ƒ+C%?½Ùß‹?øB;ëh™?÷ž§ªÿH?î+h~nšè¿äIî*ëf¿æWð}ðÇ¿åâK^Τ¿ï°Ö+ñ'¿ïý,ÆAGNbllOV 239.7?uÛæ?¨…`-}?¥ÔȤâ¢?¨…`-}?âžò3Ž¢Æ?Ì­<VÐú·?Ú˜âºu?Ì­<VÐú·?ì`Í¡DD?¨ì²"&t?¼ù'õÝߑ?¨ì²"&t?æÑ nÞ?¯ÃWn?Ò]¿#ýòE?¯ÃWn?å='J닪?Ç|0ýùÀv?ՄÝj(è¬?Ç|0ýùÀv?Âß|ðÊ
®?ÊI;J‡/?ëH ÃÍ}T?ÊI;J‡/?çÛqþux?µ\ÖçÌ»?ÐIß?µ\ÖçÌ»?Á÷ÁÅ)6Ò?§åºu?ë'Žµ²K?§åºuMIXED4FGL J1926.8+6154?âý˜¸"Qš@3¾š^»w:À9ñ\Ï
ðÀ;Îm=ðüW@Ã@7ü?üŒ•¿ðEx?¬« Ðg?µÜÃdïû@|XƒNÔy@>C">™C¿ã`䡪µ ¿¿öÔ]9ìá¿ÜðÄ£ÉH¿Ør/ÈD§Ð¿Ûwp#ÿc£¿ãZã±àbAGNbll3FGL J1926.8+615487GB 192614.4+614823?ïþL	 ˜¯?˜ÇýÜ~?+?k×LeÄ?˜ÇýÜ~?ïïî-*í?d->c}Qß?`ýÔ4ëZ?d->c}Qß?ïïé2Ò?X©Þúâ?`àÄPF%?X©Þúâ?ïó|u,¹?<¸.Zš±?YrSì©?<¸.Zš±?ïýÈëkÉR?(çB†ò©Ô?1¸£€‰†¬?(çB†ò©Ô?ï¨zÂÜh?ógy"#?…áO‰×¹ù?ógy"#?ïëÝúÜ*?pož	Õ?d"ý3ކ?pož	Õ?ïÖ¾•Òd¼?`jyq‰o?t µQÛ?`jyq‰oAGN4FGL J1927.5+6117?ª‹:!&P@3qí9SÞ¤À9d²<'ÎÀ;îQ°Ì¼@s7ævA%@ÞÄK?¬l«`&Âs?³"ÁO"ç@+
=²é@
¸`Ú
x?ï÷náàb¿Û&¢+8'ï¿á½< —¥#¿ã;©p¨¿ä{`H•¿â¢^d9eAGNbll3FGL J1927.7+6118S4 1926+61?ïü"Þ ²'?P((9nYz?;Ù
Õön"?P((9nYz?ïîŠP•2›?ct£^m4?au¯¤†Ô8?ct£^m4?ïa{?c
–ò
?apHÛç?c
–ò
?ïÕQ[šãú?V4Ÿ;fÞ?uWR1.*ö?V4Ÿ;fÞ?ïùi±cT?CY¦©ëR÷?JXÂ
.Û?CY¦©ëR÷?ï©!ðÑÊõ? ­°}?…·ƒËBÚ? ­°}?ïÑ`n;F?|3~_¾ðÙ?wOÈËÑqB?|3~_¾ðÙ?ï\À—"?x6®µÛÿ¦?"|‡÷º?x6®µÛÿ¦AGN4FGL J1929.4+6146?â~rµV`@3gag#$ÈÀ:t+'~B%À<'z@¬Þoâf@$&5îþ?ώÜð±X?ÃÁ• ¹?úNêHޖ@}}¸'ƒ%?ë™.9Ï/¿ÝÖUa±Jæ¿èÚò)}¨¿Út°`Ûb¿íޥœÈ"¿ïÿ±@LAGNbllTXS 1928+616?ﭓ þŠ,?¨¿Wëb³?"›¼íÙ"?¨¿Wëb³?ï|4ÔüyÁ?'¸(è×?yeWÙÁä?'¸(è×?ïWZ@­%?‰ï9PP?•·íΗV?‰ï9PP?îkeuƒB?…¸QDà ?©N©¨§ËÙ?…¸QDà ?î¯wz?¡².ë﵂?¥Ž÷'—š?¡².ë﵂?í¡¨C4¼?·ðڗ•Ò?²ò¼À˜¦?·ðڗ•Ò?ì鰅™\ˆ?©Y!Ñ®U`?¸²{ÒÇ(A?©Y!Ñ®U`?擞Hç
Í?°°‰ªäÅ?ÒØÃn1êf?°°‰ªäÅAGN4FGL J1930.3+0911¿™»£žoÀSÛ]‰HÀ9)êFZWdÀ;ñ`®—@qÇO_c¾@8þžÖð<?ʋ ÆÒ?ÕC!ór@Êôj ‡Ê@8ú0³&3¿ëœA^ïúy?îâþgy‹Ý¿ëyIbI¡4¿èÑ[§Æƒ¿ïû•!ººÑ¿Ö‹N<Îè[AGNbcuNVSS J193016+091037?êµg•æ[¿?ʽz:iïn?Å*a¨f'?ʽz:iïn?à' o‡Þl?Ï—£d‰?ÞÜ¿ ðC'?Ï—£d‰?é$^µ~7Ð?°â1é/z?Ën…* Â?°â1é/z?盯pÆf¬?«€Ù›qî?ÐÈ¡s2¨?«€Ù›qî?àU"=*Ǚ?Õ5Æ~‡£?ßT÷…ªpÏ?Õ5Æ~‡£?¼!ߟs‰v?ÄtÏäóùÑ?ì{ÄŽÑ?ÄtÏäóùÑ?Þ8°%!L¬?»^Ë‹Ä?àã§íoYª?»^Ë‹Ä?¸?Wôr
?¥ƒ¬HM¾?ìøk~?¥ƒ¬HM¾MIXED4FGL J1931.1+0937¿Þ¸©‡Ö×À0É°·À8=éˆÅ6À;2'î"­y@ ]ꟸ?ûfÙRí
?ª­NWPôº?¸OÂ5<g@Fß?–@ò…-H?è#qߖS¿çè| åhO¿×ùÎøö÷C¿Õ¿r¼`¿Ún?¿ÜaˆE´?7AGNbll3FGL J1931.1+0937RX J1931.1+0937?ïý{¿F°?4þƒm²ß?7#'~X?4þƒm²ß?ï¤û™á4…?•›Õ,CŠ+?†Á˜àêš?•›Õ,CŠ+?ïXœÁÂ,¶?"˜¤Òód?"ìgÆ›J?"˜¤Òód?ïíô"ÿëw?Jf'#÷Ö7?bkè·1+?Jf'#÷Ö7?ïþ8wû?)¸)¬µ?,ÏÑ^‹â?)¸)¬µ?토O©C?ÂÆNпíä?³Êý"ܐh?ÂÆNпíä?ïc{;ý?"õýø²¼}?"žþpNk?"õýø²¼}?ïÐ7ÈÄ)?e
Þ3ØAÇ?wä|Ü?e
Þ3ØAÇAGN4FGL J1931.3-1556¿åƒEßÀ/¾PÅë1<À;u–²^Œ}À<Ú.Íû¡@ "´+?û=\ÿµW?Ù6¬Ï×CH?ëpý
':@¹ÿ]BÑ6?ÿ¨C0¬E¿í"½«;X¿êº¬(©l?ïó€`°?¦°×½…uå¿íxa"·¿Õìò\(téAGNbcuPMN J1931-1558?îyŽÛê;?§¨9öjÚ?¨nweuS?§¨9öjÚ?êïqøڌ?ÈV?û‹?ÄCæ8•Ò?ÈV?û‹?ìc4
óñ?¥ÉOq…½ê?¼æ_ߨ`v?¥ÉOq…½ê?êHCÄ-Ÿ?±ª«ú?-?ÇÞÞðïI'?±ª«ú?-?ë†"ûœ\Ü?¿)§â:Oæ?ÁçtŽŒ?¿)§â:Oæ?â@+i:V?ÔCÀügÁ?ÛÕ©-‹T?ÔCÀügÁ?éìUm'!"?±àq‰%?ÈNªI·{y?±àq‰%?àãòycï?ÆQLÝÃ?Þ8
ç8"?ÆQLÝÃAGN4FGL J1933.2-4539?á¡ÞÊPE¾À:	¥e¶šÀ9Ð]ÿ—¸À<3Ð$ër@'.ϏÐ@Ïf"‹?·èÞü$SF?©¦>(ëÃ?íÀ‰þ#r@
ìª``ö¿Í…ÁµíbD¿å¬°Í'Åj¿ç³:¿ïn¸¿åíLŸ¿ì¬•à–¿ïúï,DAGNfsrq3FGL J1932.6-4537PKS 1929-457?ïý'~ÂJ4?+°p°Í(ñ?3ì®H'î?+°p°Í(ñ?ïó¹\úÏ6?li¾{†?XF‹'ãM?li¾{†?ïâ\ÒžË?iü%ŒúÍX?m£-´F­´?iü%ŒúÍX?ïý¿ºPÚt?!Ú\
ðë?2,wã9#?!Ú\
ðë?ïþªòÌ*?- ½z«m?/EP'DåÓ?- ½z«m?ïÜp˼xä?u(qîÄÁ(?qǚ7!Û?u(qîÄÁ(?ïàÄ<Á?t¶;Åá(?o;é¦?º?t¶;Åá(?ï÷xŠ³Ö9?CšÚWä3?QêaMÝ?CšÚWä3AGN4FGL J1933.3+0726?íxî ï†ÀM;€ßŽpÀ9!UŠv(À;½=1¹¶p@ ß6<ýâD?ü`¬}¡ìN?±4è%ü¿?­M	âÆ£?þ(³}pn@ì{"`'?ïÿÄ;-Óx¿èkþ‹‹¹Ý¿Ú®(ýân¿ÔpŸÌä¿Þ¾"¯<C¿Ùyª	bAGNbll3FGL J1933.4+07271RXS J193320.3+072616?ïýì‡}7c?%¾	m Iò?0›ÃsŠ™ø?%¾	m Iò?ïÃ/ì ?ƒ^c¹<?~h	꒘?ƒ^c¹<?ïãU6µ–?sŒ seÆ?lªÉ°tx?sŒ seÆ?ï¸){¬ý?hIbSð?ûµŸ\ò·?hIbSð?ïù²®
i?H´xÛ¤Vð?I5HZ$´?H´xÛ¤Vð?îdߥ?·?Âc¶`?©²ã–?·?Âc¶`?ﺳË|ž??…Ü•Ë6}H?S
yØ^?…Ü•Ë6}H?ï9í[&†?…9̱GUí?˜ÂT V§K?…9̱GUíAGN4FGL J1933.9-1025¿ïüÃ~*¹xÀ,;}æOUÀ:™Á•a%µÀ;¼,k˜Õ@VK˅yý@Û{Òv?»4‹"'Å¿º¦ƒŒçÚo@Aâ"Ÿ@†Õ/ò¶ì¿Í™—@MøÜ¿éoÜfÃË¿í—Ù¥ù#m¿Ö
‡­ÞÊü¿¥K鞥Ù)¿ïÿ•ÂûAGNbcuNVSS J193349-102530?ïðe¨GÔ¢?}FsE^¼?_4¯â›ð?}FsE^¼?ï¸%³˜É:?jD±#½¹?ö"$t{j?jD±#½¹?ïˆãù[˜z?Ø-@9ˆ?Ç—ëÕ¸?Ø-@9ˆ?ïúÍdˆ{ö?>Z"^er?DÊn]ƒm?>Z"^er?ïYþ–÷*?"öšjhÃR?"À-89°º?"öšjhÃR?íð¸ÓØï?¹É¿•ñ]?°z9d_,	?¹É¿•ñ]?îQÏ´™áN?Ÿý¸Ÿe­Ñ?ªã²h!?Ÿý¸Ÿe­Ñ?Èz?‰ö`ußËÅ?Š÷ô?‰ö`ußËÅAGN4FGL J1934.2+6002¿çøÐòSøƒ@25Ôèû½À:ç|ò™åðÀ<«Þ7X\@ uҕ¹/?ýo"èbT‰?Á¾BuE|?ÍD<ÅÙ«@Ã$­^r?ù(ǬÒ['¿ï}'›x—?ïÿ˜k¥k?§ÿÚýMY`¿Þ)¡"I¦<¿å?4(%¸÷¿á9âyÝ;°AGNbcu3FGL J1934.2+6002GALEXASC J193419.64+600139.5?ï̉	Jú?u¿žãâO?yÿ»–×b÷?u¿žãâO?éÉ@	ì?Ƴoˆ	`?ˤ۲ÿØN?Ƴoˆ	`?ïI#""-/?'*FVyÔð?–ۍŠ
¾?'*FVyÔð?ëE{à <?ž´¹Tó?ÃÞê?ž´¹Tó?ïmñ_Š?"ã`…æ?'AÔ˜¶?"ã`…æ?ÖdôÑ?ÐTJÿq~Œ?äýÍõ…—s?ÐTJÿq~Œ?ío½yêôø?¦L<©š?´'/Ìq>?¦L<©š?Ù%ÜÍ9Èè?¶û¸ÙP?ãm™cŒ?¶û¸ÙPMIXED4FGL J1934.3-2419¿èÏmͧ¬ñÀ3Ìu_þmYÀ:¸£a™xÀ<psT‹r@!	L;P?ùiU~·–?Ë!Õþ#ÜÔ?Ò7A_ƺ@к%*\@U'•ñ‡¿ïÛ>ê÷Z??ïù> #Ìc?ãÇ¡A(¿¿ØáŸÂ¨†œ¿ãǂÀºí¿Ù‹n]«¬ÂAGNbcuNVSS J193412-241922?ïõ˜"T5?QSA?TÏáy_?QSA?ï|¯eÞ¬? ïöó¨3?jLÁ'I? ïöó¨3?ï­óº'$Å?€¿zÞ©R?"ƒMø^á?€¿zÞ©R?ï3†}<µ?|{?™0_iX?|{?ïßkèRÝ?oã{-©v¨?p@IóÉMØ?oã{-©v¨?ì¯ñ»L?Ã}"«HC?º‡ïr%ž?Ã}"«HC?ïs'o" ?-DºLË?'²hÿ?-DºLË?íÔ)ï¬d'? @omâ`Ò?±^°'œÛv? @omâ`ÒAGN4FGL J1934.3+6541¿ïÿœF-r@4RmzVÞ3À9ËÆ<ÓGÀ<J<Q†Û@ߝâ)@/¸¿Þ¨?¸öç?Â,ñ$ÅÝ@¬ž#lÓ@[µ³U­¿Å\ÿµW¿èOÉkï<¿é³^™‹¿î‹1¬Jv¿ïò<'Î{#¿È³çcQAGNfsrqTXS 1933+655?ïþ¡À€³?&6òûF?%ãü¾h»?&6òûF?ïô}©+»x?\=ó.Ï	?W­['Ïâ?\=ó.Ï	?ïÏÙ]:)?w"_¢\HÇ?xQr¹²ö?w"_¢\HÇ?ïÿ"·®c?¦âŸÇa?Ò/kgÝ?¦âŸÇa?ïü^ˆ  _?AL9L9?=½¹îZd?AL9L9?ïÅfB€7?…ꃄû"?}LÞð°Àž?…ꃄû"?ïsÄY6?Œ@Ä¿'Ïb?'‡tÜ~y5?Œ@Ä¿'Ïb?ïþ[½7zã?$-hƒ9…Ì?*D+–mR†?$-hƒ9…ÌAGN4FGL J1934.5+6139?ånãM Ot@2Í=B€®À;hIóiÈÀ<¾ÀÕGő@S>€ï(Â@è"»ìª¹?Ñ*—ëè?Ívñä^cã?ü4#óûÿ@æüõ‰"¿ïý–Þÿ)k?ïÿËô_¹¿Ú#½l²†¿è}}`ݐ¿Ú)À£s¸	¿ïÿG=¬2ùAGNfsrqGB6 J1934+6138?ïú½zÁ´?@KÀ™i?E
?Œ1;?@KÀ™i?ïézÅ‹†?n÷"´Êýá?f…:µ[2«?n÷"´Êýá?ïÎO!Œ}ã?sÇÉü0Ä?xØo%ÓRf?sÇÉü0Ä?ïæ…n›-?QiP\¬ä?izéPÌ+S?QiP\¬ä?ïö0¾V#?S!‰ž—Ù?Sžƒä՚å?S!‰ž—Ù?ï…<>ìò)?•;p–Ï»?Ž°ð:t¡ç?•;p–Ï»?ïcžo±?ŽÈvÊäI©?"œ2	ßÊ?ŽÈvÊäI©?ïcpfðO?…f`ÅL7?"žñíúŒ&?…f`ÅL7AGN4FGL J1936.9-4720?ècTvsáÀ;ޜ)¦À9¦óp.À<
—þ@ ¯K¿F&€?ûé{DD?±¿jŽ",ó?¡¥ÓÂ=v?ò¦ç•¥ï@œO3™àf?ï{ˆA'¿¾Öh¬çª¿áJÕù¿Ô~Àdß}©¿ÝÊhÙÞ-G¿ÑÛR6-¹wAGNbll3FGL J1936.9-4719PMN J1936-4719?ïÿIÛb´?ZJÒ",?vȨÝH?ZJÒ",?ïöHÀGó?VÍøÏ¿°W?Soöý:±?VÍøÏ¿°W?ïòêÏ}gp?^šã˵Ù=?Z*a_æÏh?^šã˵Ù=?ïþpx¸ù[?¡6ÈòÃ?(øw}‡?¡6ÈòÃ?ïþõÀzȸ?E›‹Æ9? £õ!k x?E›‹Æ9?ïʬó­P?˜#ÖE‡Îµ?z©†F䔌?˜#ÖE‡Îµ?ïóºø9;?c¦o²Á»þ?XŠ¶:p?c¦o²Á»þ?ïý´¬x!,?&͔ùS?2Zš¸¢þ-?&͔ùSAGN4FGL J1937.0+8354¿ïñR\]î@9ÄdE#öÀ:úôàM/À<Ì+
|À@ð?S	?ÿ"Ñ‹xn§?Ċî[ôt?Á·ƒåRT·?õA›«Â'@œ¶×Âõ?ï§W\Þ'h¿àÓC>C1®¿Ò8¢]ã`¿ÞpGüó¿ägûnj,¿çã¡àø0AGNbcu3FGL J1935.5+83556C B194425+834912?ïß_½f
·?®^t†d´?pP!4ëà‡?®^t†d´?ïðÈñ‡(?^ún$Y©O?^àn˜£ :?^ún$Y©O?ïíá^̋?kl²[ãzÁ?b¡
9/p?kl²[ãzÁ?ïµ3‰¼¤?_QÇ(¹(Ë?'¸ó.¾âÝ?_QÇ(¹(Ë?ïñ…ï¡@¶?Vð¼g>X?\ô AÌ¥¡?Vð¼g>X?ïñæ}´?{n*ÝÓ ?~{¦ô³â?{n*ÝÓ ?ïÜaëµùª?|¾mDADŽ?qÏ
fÃ?|¾mDADŽ?îý2ëî?üãn»|? /GÄ?üãn»|AGN4FGL J1937.2-3958?á6M}r'»À9]&ú?̟À99­feÀ;ÿ<ñøÖ@@8xž!h°@è÷QÕ?±‹è.ú?²n¶l
Da?úÔní¥,@ͲûÀU¿Æ‹&ú•²Ú¿ä_ÿD]Å¿èØ^›–ÉÜ¿æö)	€¿îH' XÐ|¿ïµ*Ÿû AGNfsrq3FGL J1937.0-3956PKS 1933-400?ïþ§›'? ¶Ÿ?%†O'÷ØV? ¶Ÿ?ïò°‡Or¸?ci~™šµ?Zžðø¦q{?ci~™šµ?ïʂ>Mˆ?|Ìl`Ò¦?z¾àïz;ý?|Ìl`Ò¦?ïúÍRGP?6mQ–³žë?DÊ·2"+?6mQ–³žë?ïÿ:k>p?scW­hy?²ÉÅ?scW­hy?ïÈÕç}¨!?—l§aòþ?{•N:s5?—l§aòþ?ïÅØ֊)©?•^L—­c?}"Òøoo?•^L—­c?ïë‰tn£?\ol&sL?dv‹‰èú?\ol&sLAGN4FGL J1937.2-4217?¸–p±
QýÀ9óôým~‰À:ŒÆˆåí/À<pŠ:N@Mš{õá?ÿ ö4¥#;?Æ'7RQ±?ֱñðþ@
U°†E(ÿ?ø6+|s?ïsþÕ]•¿àñ
™¶õË¿ØŸ"ðoê¿æ¿ÞNÕP¿ëV&x¡Q¿ðAGNbcu3FGL J1936.6-4215PKS 1934-423?ëà™q;è ?Á صÑm?À}š;]?Á صÑm?ëHÑ274Ë?Â|M¥Çœ¯?ÂÜ»7#,Ö?Â|M¥Çœ¯?ë\–j©ÛË?§éµØí×?¦UXÕ?§éµØí×?ìÚd»?œ[¡>éÁ?¿ÇÉ,Ú)?œ[¡>éÁ?æ»ËMP?Ñ^øJ¡[Q?҈hÅÍe_?Ñ^øJ¡[Q?Ø#R-QûS?ÑÐyÁR\?ãîVéWW?ÑÐyÁR\?Ú	˜¦eÁ?Á¯š]Ÿÿu?âû3¬Íz?Á¯š]Ÿÿu?Ü/ÈåY?µl†$Tš¢?áèp›S?µl†$Tš¢MIXED4FGL J1939.5-1525?âv#‡05À1säXÍÀ:l`´u½òÀ<ŠJq=Z@¹UÐ-@ò…fîW?ȳ¤‡´??ÈÛؘÝÜê?þ06(°ù2@/~UñN6?ïá8ÿûÎB¿Ã
3µŒ¿ã% ¶Xí¿ê(ƒ¬ÈJ‡¿Þ.û–
óß¿ïÿÿ" 5•AGNfsrqPKS 1936-15?ïóBÇˆÀ?hÒÉy¥Å6?YzàDóâ?hÒÉy¥Å6?ï݄sdþ?wRWïHk?q=Əéèø?wRWïHk?ﺨÓsÙ?xÊ®¬Qµ[?UËCIÓ¡?xÊ®¬Qµ[?ïùü@ø©?2"°k|ÏÑ?Hÿ³ñê´?2"°k|ÏÑ?ïí (áÂõ?c9ÚPÊÇ?bß×Wöz0?c9ÚPÊÇ?ï3©Þ"Ò8?¤žw&?™ŠÄ/=†þ?¤žw&?îi9¿`~? \-Õ~·?©lovC*? \-Õ~·?ïç"nv&?[M;Š)@?hl'³"*?[M;Š)@AGN4FGL J1939.8-4928¿ïu‹%@âÀ;äÿëJwÀ:…¯	ëÀ<ƒ€Íù¦@þ£NÏ@~â¡Jh?À(ÁÕ¢ß>?¤3Ê7-?怮¡=§Ö@¬¶`?ïØ5jÀ¿å+îÑ"2¿ç$aß(ì¿ÐÕbÈw(¿äÆ>QÊM¿â™ДØjAGNbcu3FGL J1939.6-4925SUMSS J193946-492539?ïþ«ï²ï?QÑÀq?%AïrÍÖ?QÑÀq?ïô³§ëJ?imû(PfU?W˜°)lÐ?imû(PfU?ïø~Õ%¿`?COhJ4DÒ?Nª'$ô?COhJ4DÒ?ïü~zH4f?"—fuj9T?<-¢"-?"—fuj9T?ïþû4X&?ÞLçC? L¸µ˜?ÞLçC?ïÚÒâÝÓ?zKdŸï"?rö–q´^Õ?zKdŸï"?ïøò'òkË?\Ú"ә	œ?L5ó0¡Ç'?\Ú"ә	œ?ïõj¶_ֈ?B§~ßÊgõ?U*"PÑ?B§~ßÊgõAGN4FGL J1941.3-6210?­›H4;	ÛÀ=‹*{ԌµÀ8	j#ŠHÄÀ;½G²Jk@ÚN#yÌ@͝€Ú†?—ËÄLJ±?±­­ê‰@»Šãq*@hŸô|"%¿Ä|1>fm¿â΍âVKç¿æK<>t°¿å{f¾%7¿è-••¿ì®Ö­ _AGNbll3FGL J1941.2-6210PKS 1936-623?ïû£lë*?8tÙOW?Asêû²›È?8tÙOW?ïñô®µú?kRݎ¿`?\¢Ñu+è?kRݎ¿`?ïÛÔt}«?trr}Ä?rÆ]'E?trr}Ä?ïÿ˲p€>ð¿Gõò=>ú&ãL§µö>ð¿Gõò=?ïýXûï¥?.;ŠÒ¡n?58!֗$Ý?.;ŠÒ¡n?ïÐ4V¯ö9?ˆF_/Ç`?wåԟçÃ?ˆF_/Ç`?ïßLé_!?z™4=xN?pY‹e
Ò?z™4=xN?ïÿ˜t‰|?9¦½Ô8^?	âÑìLÖä?9¦½Ô8^AGN4FGL J1941.7+7218¿êwìwPÞ.@6©£Ò؀À:J¤ˆàä²À<¢—o@Í Øè@|lb(ê?È°`¢|?É2ØÅS†»?þ0¨ú_­@Ÿè)Ê~¿?î¼#Òm¾¿çk6#¨|¿èÏa!Xi¿ìn	"&¸Ñ¿ÔÅ
á…k¿ïÿ]þ¸Ø#AGNbcu3FGL J1941.8+7218GB6 J1941+7221?ïûÊö;u?DÝ.Ž7?@׸gdu­?DÝ.Ž7?ïô‡éeV=?[¾m›ßN?Vð,ʵ³?[¾m›ßN?ïĜÇBì†?z
m`<î?}±œ`™€ï?z
m`<î?ïþ?FÎæ?Vuƒò1?,•¦tð?Vuƒò1?ïþL–Üzë?0xý‡Âß3?+6•nÀ‰?0xý‡Âß3?ï˜~%tÚ?2ðÉ?z1Àî¥k0?2ðÉ?î॔¤'F?› Rá?¡õ¦¹&wš?› Rá?ïõ}'þ®?I$ìè5¼¸?U±¸SK?I$ìè5¼¸AGN4FGL J1942.1+4011?Îhüe85s@ ¯'Àa"À:¥]òú^À<^úaZŽ@µÈNbä@õ‹$‹Ðƒ?Á7ÉðÏ`?¼2^½¶Á?úƦå²@IÊS˯?îOd1¿Ôʍ'_d¿ã?Èl뻥¿Þ°¾ä¬½c¿îÈi[
lÐ?ØÕÔ]dßÿAGNbcu87GB 194033.4+400351?ï÷[r'ËÝ?kw¨@¿?QI4¶Vn?kw¨@¿?ïè~-¤ËH?rüiR>
D?gÒ–MÿN?rüiR>
D?ïe‹ÿ
wô?eÈËz+.?"N€¹û?eÈËz+.?ïîÇê1Y?G@Æ}("ø?aè8OFý?G@Æ}("ø?ïòùn?U]qÆOê?[Äü ô?U]qÆOê?ïOŽÒó"?¤Fá‰8?–>ã鿏?¤Fá‰8?ï@ûìJ?]Uç*V?àšª¨Å?]Uç*V?ïÀU'éSì?pa'>#Ä?Õ>xÈ&?pa'>#ÄAGN4FGL J1942.5-5827?ì-"J
nÀ=rˆXÿu—À:ÆGœvìÀ<'§4ŒÏ‡@ü HtãØ@D¯ñ¥Ê?ÈA¡µòÁ?¨ÆÍYd >?áz`ƒÎV:@¨L!Á›Á¿áë¶!d©£¿è¹> #Ìc¿àŧ߭z!¿×šFÓ#(#¿è?`Ónu¿ïÿÉ¿&FAGNbcuSUMSS J194224-582824?ïüž¯œÕ?7<Èðø??ë*i5Ó?7<Èðø?ïô®çoÌ}?Wž&¤`?V¢1x]Ø?Wž&¤`?ï鬋±
?iH̍7è?fSt_cû?iH̍7è?ïú×Ɣ¾,?.>YQH?D æ3·ý²?.>YQH?ïôþ~Âö?T>­	l÷?Vøâ¯)?T>­	l÷?ïÜäóñ:&?s"HØ$.Š?q†'¯A?s"HØ$.Š?ïÓÜòšøÐ?~ŽqÛ*+Ï?v†¼"º?~ŽqÛ*+Ï?ïêNLõ…?VòS%‹9¸?e±â·*K?VòS%‹9¸AGN4FGL J1942.7+1033¿ÛÀN~'Àsºc=¼úÀ8'%³ïáÀ;\Ì.A\@ K媔=º?ýWo£&
V?¡D{@N_ñ?ž@}@¢?ý™œô˜@֛Ž¼Eì?à@%‰ýDd¿ÓošÂŽ…i¿ß¢Š# ï¿Øae?õ¹U¿Þߟ!î½8¿×Õó¼ûžqAGNbll3FGL J1942.7+103387GB 194024.3+102612?ïþ<µ¬¹v?ÌsmôµC?,4¦ª>!?ÌsmôµC?ïÓ…
›t?¯±°%?vw=†@Éæ?¯±°%?ïÏåÖ!ú?'q°Óå?xz
P?'q°Óå?ïìÀ``pŒ?T«ÊÆ"¾»?c?ŸœÏÄM?T«ÊÆ"¾»?ïù÷õ'ß]?BF&Ätå¯?H )á1Q?BF&Ätå¯?îÎeæä¦?¯QFˆi_Y?£¡–""?¯QFˆi_Y?ïÊǐ'¡í?ƒÌðvÞ£K?zœ7¨À­u?ƒÌðvÞ£K?ïá‰å=ÿ?d%È=PUs?nþuÚ)Y#?d%È=PUsAGN4FGL J1942.8-3512¿Â"/&–îÀ9!zg¥*ÇÀ:˜£ÇðÄúÀ<7β€m@ôÃ@Z±'Ýãv?Æ-Èe4L?£"k­"8?ÞÜþ3!@@
2žb×?çQj‹¿ß]Ò®Že¿æjußÖó¿Þe¥
æãϿ֘…·d†¿ìƒ<àÛødAGNbll3FGL J1943.2-35101RXS J194306.8-351001?ïïJe b˜?rÐs¤(E?`µší[×z?rÐs¤(E?ïåT.;¸Ï?wʓìh}?j«Ñׅë?wʓìh}?ïÎÕívªE?€'=óÁ.d?x•	SÉ%W?€'=óÁ.d?ïù0£5úŽ?0ík»?K=t2·wM?0ík»?ïêiâ$Y?n¶sé_–?e–½Bÿ¤?n¶sé_–?ï
#ȏ®è?©ŒÐÁ°Ð?ž»†êš‡
?©ŒÐÁ°Ð?ï°ÌaÔ©?‰pÑ"j™?ƒÌçÑ«¥?‰pÑ"j™?ïäBt;2¨?\ëÚ§¢?k½‹Ó럀?\ëÚ§¢AGN4FGL J1944.0+2117?֎{׊s¿õ
WqÖÝÀ9Ÿ©,£ÍÀ;¦I†[Ï@#Lo'*;h?ô…UÅ.rÚ?Á`Ü8Ё?Î雥"c@Û£)eT@~¿[5z¿ëgÑÀ§zƒ¿ïé†@÷A?ì~ò¹Æ_Ë?ïýßÿ¯x(¿ÆØB¡»&¿ÎÅͪAGNbcuMG2 J194359+2118?ïRÀ"…2¯?©­ª3úì5?•§írÉF?©­ª3úì5?îÉOp?°EZ­>ŸÊ?£nk
W;?°EZ­>ŸÊ?îøáö£¤?'nÙN? qà˜Ž?'nÙN?ïˏ1Ù
o?pX-ˆåDz?z8gèäU?pX-ˆåDz?í•Xté¿?°ê½ywÚ?·;U: ä?°ê½ywÚ?êðRJGe?ÉaKÌ~•ª?Ä>¶Öãžm?ÉaKÌ~•ª?ìòäØ¡8?©Â4·OŠ?¸hÙ9@F?©Â4·OŠ?ïXÛ8ug`?˜­üÌ«?"ä˜íãwþ?˜­üÌ«AGN4FGL J1944.2+3921¿Òâg–ð¥x@V#ˆÀ:5ƒO«8þÀ<+øàQ@>c†ã£?þG.¬?ÀyF¨Zý}?͐ÉE.@ßkã}é:@%ˆà%?ï¨ÙÞ-Ga¿Ô¿·%Á¢¿Û7'"Yœ)¿Ù ºKâ¿ç0²ð'´{¿è֔aKtsAGNbcu3FGL J1944.1+391987GB 194223.9+391242?ïŒRV9¬?‹`›´–œ?Œëj'æàÛ?‹`›´–œ?î9žèõ»?²&[n"¹?¬frgRT?²&[n"¹?ï¡æLO¹Ò?ƒ`_/H??‡†lè¡ï?ƒ`_/H??î>i(§Wâ?ƒƒ',&;`?¬mröÌã?ƒƒ',&;`?ìèÓÙ[{|?µðWpž0?¸¹a5'¡?µðWpž0?åG21^$?Ñ«çг?Õq›C¶þ?Ñ«çг?ë¹#B'å?®¨Slo²?Árõôl?®¨Slo²?çz"8'õi?®N¥·VR?Ñ
÷ŽÜ.?®N¥·VRAGN4FGL J1944.4-4523¿Äî'VSk.À;ãü–þµÀ:òŸÅ,ÅÀ<aV"@!±ð°.\?øœ5Ċß?ÃoKè5Þß?À¤AhU(ü@³;–¯Ž@K-Kè‹Å?ê9!°:?ïÎ~T–Z¿ß€ aIq
¿È"CÄOû–¿Éö$_ó/¿ÓóBWhrAGNbcu3FGL J1944.1-4523SUMSS J194422-452333?ïþE%Š?$èñ‰iå?+¯ÎùýV:?$èñ‰iå?ïí²VÙ½?p®
VÈ?bMäëÂô?p®
VÈ?ïóE¶²H?Mƒ>;Ð?Yt'\70<?Mƒ>;Ð?ïöCÂç4œ?@Ò$×Î	?Sxyç_8·?@Ò$×Î	?ïü
žÙ8Z?@æI'Í??«­gˆ?@æI'Í?ïÉ˅Ïã-?ƒœgÛ?{=7ªÑy?ƒœgÛ?ïëÄì{
Z?o$ãF±IJ?d;®0ö?o$ãF±IJ?ïábš÷4!?bɁ Kƒó?ndÑÒf?bɁ KƒóAGN4FGL J1944.9-2143?îÀéx:_‰À5ȊGìÿÀ9:._ŽÛÐÀ;݉à¾ò@ di¾µ‡â?üYÝÁç–?®JícÙª?«>Ÿ'ª?ÿÛÇ4Ý@y؜ŽÁy?ïíj Ûç¿Ñ*Ÿµg€¿Ùêã"ύǿԠº $x/¿á`‰þ#r¿Òr¬ÅÆHNAGNbcu1RXS J194455.3-214318?ïþÇĂÙí?[GÙQt»?#ƒ¶ÜÈ©?[GÙQt»?ïåËÂiO?vŒœÖnòá?jì49w(Ù?vŒœÖnòá?ïæÔ#Yˆ?pÁ¦8]?i+ìéX?pÁ¦8]?ïûI–½ò?/ËH'%Gi?BØöDvÕ?/ËH'%Gi?ïþ<wè?*"Òçšr?/ü:0Ñü±?*"Òçšr?ï?"sÜ_?¢ªj }{?˜qsî?¢ªj }{?ïÞÕ;:¥?vT+ËáR?p•pÚӉ¡?vT+ËáR?ïù·%"ö?;«üš½[?I#håǚ‰?;«üš½[AGN4FGL J1945.1-4007?ÒpöŸ{}FÀ:Þ*<êlÀ; κÖ¨À<¾€íÑ)S@éé%Lk?ÿ^½çX?ÑÑT›ã Ï?àùJn¹?@ê¢þ)q@
u?Öڗ¼¿ïÿÐ?sŠ?ïýáAÎ×i¿À¸™¹úã¿â–Æ ¸Ç²¿ïÿo·HJ?ïçh5'‰AGNbcuAT20G J194519-400557?ï÷âLÒK?]éOtê[&?P;fy3·ã?]éOtê[&?ïðÙ¸SÕ%?d!y%¢?^L:%F?d!y%¢?ìý'첓?£ä:jžª1?¸Ç1^ê?£ä:jžª1?ïñØ©
6 ?NÈ*\É\?\N­©›@J?NÈ*\É\?ïôÕ¾I7"?aփ§ŽRª?VTƒÙë%?aփ§ŽRª?ï°IÛ[d?"át¯"?ƒí¹a•$?"át¯"?éµÈú¸Ëí?³2Î1Çe?É(ÜÐN?³2Î1Çe?ï´½ÝyJø?v=é¢?'Ј•þ–?v=é¢AGN4FGL J1945.5-0153?ï*[¾ö(À)È
°ö­À;!C|V'´À<9.¿0@>ßôñ"@ݼfM;ó?Õÿ\÷§Â?âQýŽ5¸I@mczù›b@ÔQpµõ›¿íسà¢ý?ïÿÔqܼ¿¿‰c˒¿êDm'ºZ¿ïýibDBпàÇA<á1ßAGNbcuPMN J1945-0153?î´íèÖÈ?°ZDÍu¥?¤±!¢/?°ZDÍu¥?è‡W\)Ä?Ç#6»ÓÖ+?Í㞢Xð?Ç#6»ÓÖ+?ì(ç4#•~?¤"!Êôé?¾¸Æ^ãT?¤"!Êôé?êó÷<?ª? Ö°¡)"<?Ä1¼#X? Ö°¡)"<?诀"S›?Äÿr€>îl?ÍAÿÅ®±•?Äÿr€>îl?Óì‡òAa?Ф‹¶é?æ	¼ßuÏ?Ф‹¶é?äa:žüâ?ºp•xï?×=ŠÂÄ<?ºp•xï?Õ/tO¿‰?·<¬TÛo??åhEØ7 <?·<¬TÛo?MIXED4FGL J1946.0-3112¿ìõbÅÇõÍÀ8'ÿ.Hè§À9wQŸ/ÐÀ<	ûï»@r*$Þä@•a[dª¥?²&rÛiȜ?ƒNcnÝÙ?ѧé=›Áè@#â~å¹-?À~Õ]•¿éýaw¿ámÔº.¿Ùˆdà
—¿é:aûš°¿à;š{pdAGNbll3FGL J1945.9-3115PKS 1942-313?ïö_8'l^?RoU[Ò¾?SA5Bó?RoU[Ò¾?ïä‰ä½%Ý?v¢ý>^ú?kvbvŠ¨?v¢ý>^ú?ïÔã«¥N?x0c/ZL±?uŽ*{ùx?x0c/ZL±?ïå;$CV?YÍó°ì½r?jâÅ	€?YÍó°ì½r?ï¯Öqç#?€Tr陛¤?"
c‡?+?€Tr陛¤?ïMí¿i?'?¤"4ˆ{l»?–BHÿw°?¤"4ˆ{l»?¾»DÃ?‹åðùì"g?™PQ.ÏT?‹åðùì"g?ï½8Î0W¿?ud¿ÑËg?€±Ìjû??ud¿ÑËgAGN4FGL J1946.0+0937¿èh£Ì'./Àõ@‰]À:Ucé´d À<DF€íÑ@ D§•ßc@ÚõýG¾Û?Áò¦%C0?ˆäŒ1&=¬?ȪJè\@O7 «1¿îAÎj[¾?êÞæu¿ãŸD(y¿Ù]$~£²¿ã·/+H¿â(TÐAGNbcu87GB 194328.9+092856?ïõÌțå?OÙ4Î
?Tfn±%ä?OÙ4Î
?ïÇâþ΍Ó?'bœh:*æ?|€¦w†F?'bœh:*æ?ïßß®÷á?kí^øfä%?p¿1{r?kí^øfä%?ïÍÕy!\¥?`
Ïú[†?yC…O-?`
Ïú[†?ïÔtÜuâ/?q§MʀDz?uőǬM?q§MʀDz?î«×*¸'?ª¼3gp?¥BUSô"?ª¼3gp?ïµ'¤á?…fb¸ç%?'¿y×I¼?…fb¸ç%?ï
÷±Ê?Ž:
ę	—?Ÿž~8rÀÅ?Ž:
ę	—AGN4FGL J1948.3+1207?ïùõdúMÀ.Ü ý¦‰À:ˆ­Ú™>*À;ô"ªlO´@±)bNÿ—@=sãýjú?҉Uê`o?æ
²
©§@/'…€!@BZœ¿ê?é£%¿,P@¿ã÷æV
ΐ¿àüÈþau¿êèNòÄ®¿í¦i³Ê¿ïÿâ–é¼AGNbcuNVSS J194814+120645?æAÏT€N´?ËèèŽkµ}?Ó|aVÿb™?ËèèŽkµ}?é|݃©BY?ˆïÙ¨c?Ê‰ñZöœ?ˆïÙ¨c?êˆðʶz®?­åóx'ññ?ÅÜ<Õ&F?­åóx'ññ?êÒþ­š'?¡÷ $g?Ä·üI•ö?¡÷ $g?ÒúX þm?ÈñpcH?æ'Ó¯ó€É?ÈñpcH?Éßݨ´Œ?È"Ì%æw ?éˆ8ȕÒÝ?È"Ì%æw ?ÖYIK½1"?¿<½œ>uÃ?äÓ[Z!g6?¿<½œ>uÃ?Õ–o©Â?µ¡Í­òß?åtr4È+?µ¡Í­òßMIXED4FGL J1949.0+1314?Ý$T¶zÀt/è%çÀ9nç¼<[ÑÀ;˜Çÿ²|@`M"ÃÌ@ïÃqÚ7ï?ºþy×ÝL?¾eà¦@æ<$s|Ï@›®] ïú?ìö쀜GŸ¿ãÿ!é^ÓË¿ãtßp=½¿çIH¾H¦¿äé0&Ž¿è¥
±3êAGNbcu3FGL J1949.0+131287GB 194635.4+130713?ïÌ¢¸|2Ö?°$ïȁ6í?y®£ª‰<ê?°$ïȁ6í?ïxÇTÆ^|?—ݬ0.¢Ô?çcĔ}?—ݬ0.¢Ô?ïÛdsXM…?sµÁ%KT?rMÆO¹µq?sµÁ%KT?ïæ&åòä?|1vjôú?ã;Ò"?|1vjôú?ï"ã£íŸD?›X)yÛj?›£‹}$­"?›X)yÛj?ìY¸g²c6?¿£b8aùÎ?½2<ÂlæL?¿£b8aùÎ?î"}XpZ? ¢îùd³È?§-Ø)i? ¢îùd³È?ê#‹ŸŸ²?¦eλ	añ?Çqùс9?¦eλ	añAGN4FGL J1949.4+1247?ç%³HAbKÀ©Oð\À:‹n}ŒÙÀ;¹rl.'@ŸœBk_u@gFBÐ_?Ð1Ñß0Q¬?ÂÊ7F=Q?ô‹Ëz½5€@®¡É=÷¿ïü2¶5±"?ïûçÂq¿ä¡>iÈ¿âÄî|Iýz¿å±[Ývh<¿ïþñ­VåÀAGNbcuTXS 1947+126?ïüБ)?PaŒÝ¼p?9{vZIò?PaŒÝ¼p?ïÔI"*CÃ?6—Bޖ3?uÛnӀƾ?6—Bޖ3?ïÁnÑ*:Í?|dL›½ð?H—T5-?|dL›½ð?ïõ"K]Ò?@×uðÿî¼?TÙhó{»¢?@×uðÿî¼?ïê©ùÛp ?h7ÀW¾ÃÎ?eVó€*?h7ÀW¾ÃÎ?î¯(¥Ì¾ñ?±±MfŽu?¥
u£4í?±±MfŽu?îg½Zi? P|¹÷Î|?©Ž-ÉÙ? P|¹÷Î|?ïÂ~¤9Ÿx?tÈÙñÎ?~À­Ò²$5?tÈÙñÎAGN4FGL J1949.5+7311?Áùœ…ÿ€@5ÕU>öµÔÀ:WçG¢VÀ<݂ýuâ@Ÿî)†Œ@͒tâ*,?®Ãaéÿã?¿Ú®ó׏?üØþÒ—@Nޞ†hd¿ß¿1×JÕ¿æêG1ù¿ç`N‰Ðκ¿çXjû ¿ïÿÏ=ÀTï¿â"h\૧AGNbcuCRATES J195016+731028?ïûæ9ýŸ?92RÏæö¯?@gû8W?92RÏæö¯?ïìú­cXž?b	­6=A?cRdMÊË?b	­6=A?ïé/S!1 ?Zµ€Ú¢Ï«?fЭ‡ÏW?Zµ€Ú¢Ï«?f®Zpå?e'38ýz§?€žTfL Ó?e'38ýz§?ïîÇ5*¦"?`@þþCVˆ?a8Êè—;Å?`@þþCVˆ?ï—ÿ2¥™­?ÖÝq*?Š3Oº\Æ?ÖÝq*?ï³n{w‰h?ƒñ—>@ô?ƒ$aÿ^?ƒñ—>@ô?íÏ¢è«?™Ål}¤?±‡'ïÓ¬?™Ål}¤AGN4FGL J1949.5+0906¿èæ=öÔÀ!? §?uÀ9·
Ø/×^À;ýžvx,@ X醖Ý}@€©Þ‹;?¶"ÁI–¢¿wä
¨‹R?Â
]v'Ï}@
$ô)Ýôè¿Ô"mè2Ú¿æô¸Œ£è¿çÏ
Ÿ$óÕ¿ÍHuûìÊ¿Ýqœ¥g®¿ã=ȝ"#^AGNbll2FGL J1949.9+09071RXS J194934.1+090655?ïýôr$?"­£§
šM?0_D#y!?"­£§
šM?ïØ\Ï}šú?" ¾ó«?sј7"šõ?" ¾ó«?ïõ[ï"øË?Iæ—<´É›?UH!O©S?Iæ—<´É›?ïü૦âW?#a,ØLˆ?8ú£J«PT?#a,ØLˆ?ïýŒ¼L³?+ræö?3š‰èös?+ræö?îé!âRðé?°9Þ£,ù?¡máßto?°9Þ£,ù?ïò0è'_ ?`ÇWŒ½?[ž.l'Š?`ÇWŒ½?ïøL=¬o?@UªÕ1¶?NÏ	 £ ?@UªÕ1¶AGN4FGL J1950.6+3456?×ô¨ë#Ø@&!`¢ØÀ:±îX7ÏzÀ<.ʔ
hž@!P¯ýˆ¬?üâDhå?Ó«'Ëöãø?ÁP±ˆÎ›.?÷X¨ø².?ÿG˜ÛX«¾¿ïþ9áùâ?ëa±Ë¿†"?ïü¾A™¨]¿ç(Îàù)¢?˜!ìf#¿éßÓÚÞˆAGNbcu2MASS J19502776+3456224?ïýyy`?2­7NÅ×?7ì3@è8ÿ?2­7NÅ×?ï¦L¶?–¸ïvû?†lþUçÛI?–¸ïvû?ïØB6äÌ&?rJCÿIO?sÞäž
!?rJCÿIO?ïºK"§ˆß?m9§i"‰­?mØÝx(?m9§i"‰­?ïêä-š ?i\ü(.Æ0?eøý?i\ü(.Æ0?íè_{vÕ?ºƒçŒì?°½"'‰Ý?ºƒçŒì?ï^z[ˆ3b?'·qŸ>D?"0´" ý´?'·qŸ>D?︱e?"?¡;à'
?ŸhéÝۑ+?"?¡;à'
AGN4FGL J1950.8+1211?íFï‹Ã&À!úvSCtÀ:دYÀ;ȟ·ÀÌ@,Ža'&@û
z<A?Æjt!?݂Bdÿ^@ítýØÞS@°7êê¿é°ò¡G¸Ñ?í˜{V¸sy¿ä–ù¬(è¿ç(ÒÁ&¦¿ïÿMéDÓ¿ãÒ ß²CAGNbcu3FGL J1950.2+1215NVSS J195059+121316?Í·Øöô
 ?Åþèx}•?è'	ÂBýx?Åþèx}•?ÌOa®æ?Å-ÃÈY´?èì'"º‡?Å-ÃÈY´?àO+då¢?²VÇ?¢µÖ?ßa©7ò4»?²VÇ?¢µÖ?à>XSºM?°™"ÖB?¶?߃OX‹e?°™"ÖB?¶?'¥9ŽU¾"?¢T>Oáÿ?ïjÖ3d¼?¢T>Oáÿ?¡§Îˆ??¨D`s†€$?îîuƒ\7Ü?¨D`s†€$?´±b K?¤Wͤí?íiÓ¼2ÔF?¤Wͤí?¦Ç²S÷9b?"ö*ÕpÔ6?ÚÎJÚ?"ö*ÕpÔ6MIXED4FGL J1951.8-0511¿éÌøPߥÀ/–¤D‡À:Mqåöi~À<¢Ô«¾_@܁Ðz+@)2^!‡?Ç*ÖØ¿IW?ʘD/ùŠ@¼]\Òi@8lýv?ïö¶^Ì>¿®^‹{ž±Ü¿ä«¤=âc¸¿ã_Cý…Ò<¿ì]2K­¿ÏÛ¨ï³AGNfsrqPMN J1951-0509?ïßWøÔ+€?pöTÌ[Eõ?pTžÙ<!?pöTÌ[Eõ?ïӏ
à¥?a1Kdô?vr8•<y˜?a1Kdô?ïRF>'Øâ?ŽWå¡dK?•·8@,M¸?ŽWå¡dK?ïíØÙ~µ?FÓaLø¤Û?b'&DS?FÓaLø¤Û?ï¬VÛ.†?†Òx…Þ$?"êI&½îˆ?†Òx…Þ$?îñ÷þ÷
à?©eÝT"f­? à€!ú?©eÝT"f­?íyv_Ç ?£Wч£v2?´4M1ö'?£Wч£v2?ï²K9ÂÌ÷?pp¤|ÿ^Š?ƒm1‡
²:?pp¤|ÿ^ŠAGN4FGL J1953.0+7651¿æ0ª}þ™µ@6øäd™ÍÀ;TÍ
à-ÓÀ<±
?x@k w™¿"@pðÀÇÛÌ?ÐÙÖÀÁ{¶?̓{~% ?ø‰Z¼äø=@ã…"¿¶?Äßbцp?æ
ÇNފ¿ãxÔ'4!¿ÛŸ¯È°š¿ìô_î} ½¿­s£æ¤AGNbcu3FGL J1953.4+7653WN B1955.4+7642?ïÓå?ŠY‹?m²¯Ð÷®•?v
`)¥.½?m²¯Ð÷®•?ïÝ]û\$?p0zÛÿ?qQuˆ:?p0zÛÿ?fU?€aŒÁ}»þ?U:iêF´?€aŒÁ}»þ?ïŒ[ÏÎMÅ?j¼¿ß4 Ÿ?ŒéKƯ?j¼¿ß4 Ÿ?ï¦/†Mô?€P^2¬wÝ?†tƒûW?€P^2¬wÝ?ï4µiXß?¡ÖD¶6Š
?™iRÌM'?¡ÖD¶6Š
?´Uª?š©n—2??§Ô¼;	_?š©n—2??íja¼Í?'?žïÒ Îˍ?´¬òºÇ?žïÒ ÎˍAGN4FGL J1953.0-7025¿Çw"×°"À>–Œi/nƒÀ:PYddIÀ<eî \+z@îl"¸Œ@vg=%û<?³ÆÊ¿¬RÚ¿©§Çà	k?õÓ	AÈ!l@õdW"¿ãc¸6<Òï¿Õ'šCÅ
¿æŸ¤¯rÊ¿Þ½Ÿ
ò¢¿ãžlґ1ì¿Ø<åcœˆAGNbcuPKS 1947-705?ïûÕiåˆ?1qUF㕈?@ªW{ÔS½?1qUF㕈?ïðúû£Ù?^LTŸC ?^
£ÜÎV?^LTŸC ?ïîHà™ˆR?blÕË3ÿ'?a·fw®7?blÕË3ÿ'?ïðßìöI?C£\œtsÊ?_Ø@ "
«?C£\œtsÊ?ïõºa=Ð?G¸.·Úžc?T‹=[6NÊ?G¸.·Úžc?ïIJë‹e
?'î´*ª?}¦ŠH»×?'î´*ª?ïé|¯9O=?pµi-"‰?fƒPÔo2²?pµi-"‰?"^¾Ÿ?~ü^?SZڑèh?~ü^AGN4FGL J1954.6-1122¿Æó7kb_ØÀ3 é_ªŠƒÀ8çDŽ¥JÀ;Õ¤xð¬¦@›jT1°@YgåÂg?ª—Àâ™ú?®¬Bn~R@±!«KrÅ@¨sÿ¬*¿Ã£]<Ç¿ä%"?]ä¿çšÁaߙ¿ã(ÛPN¿çd×Oݍå¿éÅW ºJAGNbll3FGL J1954.8-1122TXS 1951-115?ïþ".<B??Š÷ð?'½E'¥X?Š÷ð?ïåäh?pÐxº¼(	?ju6 ˜
?pÐxº¼(	?ïëå0=Vð?aìjDjÔ?dÏÈ(p?aìjDjÔ?ïþ<	Õ?}Æ (‡?,>¹ûZ‹w?}Æ (‡?ïý,~8?7?48®aúf+?6œ <ò?48®aúf+?ï5øÌý@ª?¦0Œµ'
?™@æYx²½?¦0Œµ'
?ïÌ<cªí?}³
ÿ™p?yòáÕ	Á§?}³
ÿ™p?ïûÝ/ŠK?2ɽîçÝð?@‹Aâì
?2ɽîçÝðAGN4FGL J1954.9-5640¿À—ÁÄVÀ>ütÙÆ°SÀ: ó9H *À<`Ñ>K•*@ mIT1Ûo?ÿ*.!{zË?²yOa½	`¿¢kÁo Ÿ2?ñh'iIo¶@RÉÑoÊ?ïقˆŸ¿ÕŠûœ$¿åÕ¶`#× ¿Ú_á§Oe¿×LÕ[;ºì¿Ñ¿LF)¯ýAGNbll3FGL J1954.9-56401RXS J195503.1-564031?ïûÞwëÊ?7'B'R?@‡¢¥[QA?7'B'R?ïòÔMAÏ?`YŠ¡ãL?ZWeèø1—?`YŠ¡ãL?ïè¢MÈ4ã?paj͂ ?g]²PˆMS?paj͂ ?ïô¤Õëb?=îõc3—-?V¶TŽðAË?=îõc3—-?ïøCc,%?BÞð!gQŒ?NòtõrúÉ?BÞð!gQŒ?ïÑö¸»F?y$6|§
%?w¤ñ0Ó?y$6|§
%?ïæáÒS°'?u‡äÒ³YÊ?i-™°?u‡äÒ³YÊ?ïÍˀO#\?gW2uÙÛ?y?Åàmí?gW2uÙÛAGN4FGL J1955.1-1604?ïþY().À5%ð=]…À9¨èÄ3¡À<MjìÝä@ 2ót'Ý@8S 8"¬?²¼ùÅÿ(??_£Ê­à—?²~9|§›@éú8•Èª?ïoAT©P¿çPB7²ô´¿âI>¢Òþ?¿àÂkµZÀ@¿ßì.Ý
6Ê¿Éæf%ù¹ÀAGNbll3FGL J1955.0-16051RXS J195500.6-160328?ïý5r¨"?,íLœ?6Tk†È›å?,íLœ?ïé=0ëá?mác¸Ü1ô?fÂÏ2®¯%?mác¸Ü1ô?ïòÙ|úÒ?]ï6  ?ZMßH+?]ï6  ?ï÷}V†¹1?<‹†¨"¼<?QRŠ~–?<‹†¨"¼<?ïúWQ†Â?A|]tΡð?Gº£A¯"®?A|]tΡð?ï"ïô¢²P?˜ˆdc?ŽÄèwÿ?˜ˆdc?ïí}°@5`?nJ"Ü£'o?b'O§
o²?nJ"Ü£'o?ïîz†¼?PϪŸ;Ê%?a…äô÷dV?PϪŸ;Ê%AGN4FGL J1955.2+1358¿éÙº©è#ôÀAÞÑ·À9å½^šÀÀ;¶UNæíà@ÂІ×}@6ï›-îP?¸_ðU"?ÇhóÉæ¾f@
'¾}~°à@¸Wï«&?­3!8E'¿äŒKÓ=)V¿ä$"Ÿ^Õx¿æö`y½[@¿éœ#î¡¿áüŒéAGNfsrq3FGL J1955.1+135787GB 195252.4+135009?ïܞôC֑?nÝ[Ö¹Œ^?q°…þa_?nÝ[Ö¹Œ^?ïÈJ¤ˆi?‡¸·yÐç¿?{ڞowÜ?‡¸·yÐç¿?ï"1ƒ׫?ô,¦;êm?‹3Ÿ7êÝA?ô,¦;êm?ïüp¸òÞ?&3û>òiè?<z6›Ö1f?&3û>òiè?ïYfÖ£»1?•tP"Æî*?"Ó%+ˆ™í?•tP"Æî*?î'tX0\ƒ?³Š0Øhv?¦Øºx®´Ö?³Š0Øhv?ëÞuÊÙY?ª.‹Rë?À†(Ôñšž?ª.‹Rë?ïñt¿o—?LpxÝñóå?]R|´?LpxÝñóåAGN4FGL J1955.4+5132¿ì˜mŸA¤@'šoÅåÀ9†¸UFƒrÀ;ó€`°@m"M¥$g@çç†w~?¹Hw"^?¿†Ñ™»(@²¬ûv-"@õäÇ|¿ã¸×í'?2¿âüÕ©¿å›À¿èý,)Bï¿é'ìKî¿ïÿÿ&¦³AGNfsrqOV 591?ïüµE2?1— èç?:S|ÂuU½?1— èç?ïï
MGÑ?h€ÿ²Ö
?`õ²ÕÅæÊ?h€ÿ²Ö
?ïâgHŽ$?blOŒ—Áë?m˜· +‹I?blOŒ—Áë?ïùY†ÐÌ?5" âè«?J™çBæ‰e?5" âè«?ïô¬˜àó1?Pð‡ŒÝ»¶?V¦ÎFX®µ?Pð‡ŒÝ»¶?ïåÇUШ?"n¹ó¶ƒ{?‹ÆŽÍf?"n¹ó¶ƒ{?ïÁÇÏÒ?‹]ùððŽ?ºÏ|Ýÿ®?‹]ùððŽ?ïä½Ôû?\õ\GÝnð?kêC"eã?\õ\GÝnðAGN4FGL J1955.7+0214?¢tÌÝH-À*l´¿ÍhÀ:D÷m5ŽÀ<$@µÒµD@!F0¿:'ù?üïçžà*x?À«˜Ÿž–Y?·A©ÿ©&?ü\6@'¥LUC(¿Ù=ªðÙòO?ïû¨LºÃ¶¿Ð"yA4}¶¿âñÃA2Ð7¿ØßÁœ"[¿ØqMJ5®AGNbll3FGL J1955.9+0212NVSS J195547+021514?ïç˜É¿?•½Z•­
Û?hg6è@èö?•½Z•­
Û?ï|]ï†S?•à³:}Êô?tB¿™§?•à³:}Êô?ïËìD-ν?}±$Æ¥?z	Þ%å…?}±$Æ¥?ï[žê;r?w»ˆ±.֖?"Œ"±²to?w»ˆ±.֖?ïά°4?z&"mx'?x©ù°ÔøV?z&"mx'?ì"äàƒ§¯?À"5šäP?»`Øûâ‹?À"5šäP?ï,é›Ë´/?˜(Á(©Â?šb́b!?˜(Á(©Â?ìòܕäû?¢•ŸÜB¥?¸iR!þ?¢•ŸÜB¥AGN4FGL J1956.1+0234?Ø"Í:ì÷ À*EóFí$À:Æ3\MÞ°À<8x{;à@ O¥ï?ÿÂÑ¡GãÄ?Ñd£Ã"ô?ÖW»þžV@FÚhµÌ@ó¹Qoß6¿ë7¯ß/j?ïõŠ@`B`?ߺl¢ë|æ¿Ø8ÝâHßî¿è¯¯…")¿áçÀÃÿõAGNbcu3FGL J1955.9+02122MASS J19562808+0234250?ïߺ"%CÜ?s7¥:r?p"îçÞ±á?s7¥:r?ï9!֔¢?£df™Ø|Û?˜ÛßíÄq½?£df™Ø|Û?ï5èaJ?6?eùI¦"Ý?™BóÛ߃A?eùI¦"Ý?îë/Ïâ'?ƒ+ä{:l?¡MFz‰?ƒ+ä{:l?ï^5ö,?š€òîDwÆ?"9A?:}?š€òîDwÆ?ëÑÍ©&æ…?Ėµr¬ß‹?À¸É[deì?Ėµr¬ß‹?í×2tz?¢Ï×_¡?±Fl[Áôa?¢Ï×_¡?ëºýÖ@O7?­í9WN@?Á¦þÃ%?­í9WN@AGN4FGL J1957.1-3231¿ß	áVÀ;7¼ä!}(À9üŒí¹¬À<? §?u@r⪯–†@–äÛ·K[?ºò¿¥œÝ?€{ ñbê?À—Á'R)n@	œp›ôgÆ¿ê b‹l¿Éy&‡~9¿ê$º"¦¿æÀ!ß&¡¿Ýsb"^úŒ¿ïçH®ÅzÉAGNfsrq3FGL J1957.0-3234PKS 1953-325?ïÂ8‹?´ŸôóŒž?~ˆ??ãC?´ŸôóŒž?ïäñá{§ä?wÑ\^'º	?k¿qd-?wÑ\^'º	?ïµ	ô9g?'#¥²eÈ#?'½'íÞ§Ú?'#¥²eÈ#?ïýMÓÈi'?!°8©B‰?5'`q¿'G?!°8©B‰?ïö)069ß?Y‰…Jè;ª?S­ŸÕ"Áš?Y‰…Jè;ª?ï\šö?¢!+*Ð?"l¡C%&}?¢!+*Ð?ïauþ‰Þ?DŸs ª?"Ý'9OŒB?DŸs ª?ïôÕÏÅ?K;úßRVI?WÑßÓ/'Ž?K;úßRVIAGN4FGL J1958.0-3845¿všªJGËÀ<öÄç%>À8P®{¨îÀ;«Ãæg@·RO@kÉÂbæ?£jåØÛ,?ÆÈ"D"š@"Ñ»IÊG@e:ÂHº¿Ït"çÙ´¿Ü¶}Àu%œ¿ä‹ÿG¶¿æ´Ka'bE¿ìO°â‹zó¿ê$Ɔ"ÄAGNfsrq3FGL J1958.0-3847PKS 1954-388?ïŸ*xW2J? _ø.Žš?ˆ5aÙa¶? _ø.Žš?ìnPÿæ™k?ÂFü0ñ8?¼xË4¥?ÂFü0ñ8?êø²H3—Ô?¯‡³
ðà?Ä6ß1 ®?¯‡³
ðà?îígú¹$?"v&aŽqe?¡)€aL;¼?"v&aŽqe?îϼ­^·4?£8àßÆ}?£5(\¾¾?£8àßÆ}?ÙOÍ.×?Ó¥<°4«?ãpXhÿ?Ó¥<°4«?ê˜/JµÊ?°×6–/?şBÕ+"Ø?°×6–/?å xxÙþ?À	(à@it?Ô¿ÉL?À	(à@itMIXED4FGL J1958.1+2438?ëŒEâÒ•À8*»À9Â¥Ξ^À;î*ëf@!,çƒ1xH@[GA1M?»1±×(¿x}xü–'?¿Ñm_BÊo?û¢ÝŠµ%;¿ï'Yԇ¬1?ïÿ…¡•ž¿ÊÑÖâOj÷¿äWF¾*rš¿åŠ ½zIr¿ù[1e8ûAGNbcu3FGL J1958.1+2436NVSS J195800+243802?ïõÀnù©?N½¿f_ÿ'?T"&Üö?N½¿f_ÿ'?寮[ª9"?'G['^sç?†Péá7
?'G['^sç?ï‹õ³¨Ä?ˆh,¯ÎsÈ?"¦3?ˆh,¯ÎsÈ?ï*I¼—Ã?…wE$ÚýS?š¶Ýˆm¦?…wE$ÚýS?ï»ãà?|£ƒ`h:?9J±…ó?|£ƒ`h:?î]Åݼ«?¶²÷(¦9?ª#¢%.?¶²÷(¦9?îÕ«ÂLQ?›HèAÁm?¢¯Å@kží?›HèAÁm?ì@ýê.»?®EEmc?½ø®Š'È?®EEmcAGN4FGL J1958.1-0711¿ëÍeàžT®À2Œ?>À:¼áÑ@ÏÔÀ<SbI¡3Â@ +Ôíˇ@_…Q
8Î?Ç{×ómK?¨.ÀÃæ/†?㍷ä{õ@۟@!®&¿ã—ëy`>.¿è3¬jVµï¿ã†Å~ð¡¿Ó:Êi²K¿ãkùM^X¿à½ÛÍñûAGNbcu3FGL J1957.9-0712NVSS J195801-071348?ï³y.eª?¶Ÿ8µ–3å?ƒ!¹~}d?¶Ÿ8µ–3å?ïßþD~?vá'OÕ~?püÂBa"?vá'OÕ~?ïð[Èµf?r.•
F¦4?_Hà`$Š?r.•
F¦4?ïý	iúßI? ‹Fm?7´®i…j˜? ‹Fm?ïþÙõTUm?†çë j?"`§ ÐDÛ?†çë j?ï)‰.ùxã?¤ýðƧÞ?šÎÚ$@Œ?¤ýðƧÞ?ïôòÕÂa0?hX6NÑ?VT
JÇ?hX6NÑ?ïô¬áä¥Ë?IcGeL¾?V¦<¯¦¨Î?IcGeL¾AGN4FGL J1958.3-3010¿¢%õº°)NÀ:È-œñ<ïÀ95íKÈUoÀ;Ùý2Æ&@ àZX?ý&ú@£^?¯ ö° Ï?˜ð|C6Oa?ì¿ÓÀí@
íœûù¶?ïïíJ.¿äÞv]Tní¿àR0N|e¿ÒžnÀ}¿ßœdпÕb¿¤(AGNbll3FGL J1958.2-30111RXS J195815.6-301119?ïþ3p´ŒÔ?'=#ql•Í?,ÈðrH¢c?'=#ql•Í?ïã70Tê?zºðˆ"Î?lÈÏÏ¥?zºðˆ"Î?ïä\ÇQ?t#"™§sÞ?k£~z?t#"™§sÞ?ïøèý'ƒ?;"-è)àæ?L\	oE ?;"-è)àæ?ïûD­À(`?Bþ-u䝡?BíIˆÎßæ?Bþ-u䝡?ïeN̟^?¡cÈÂüê?"V&l??¡cÈÂüê?ïàå¡…?y¾ÿ¾w:?oêáÙw?y¾ÿ¾w:?ïõ	¢>+?Gk¼J`V?Uì¼¼zB?Gk¼J`VAGN4FGL J1959.0+3844?â@ȂÃÇÉ@%/<-­¸À9Ëx²Õ«À;'š0˜N@@q€»QO@1^aµ&¾?·¾Þ!³Ú?ÓUÃW@Ü
²p*@>3U—â	¿ÛW4ó&Ô¿äL#ú±¦¿çT¥ÿX:¿äô1•¤A"¿ïàñ4ˆs¿ïÿù³>†AGNbcu3FGL J1958.6+3844LQAC 299+038?ïŒ"´Q£?Šé•È€l?Œû^ȜÃC?Šé•È€l?ï{i15ÆÐ?'|‰‰QŒ?'ÙáÞ+ð?'|‰‰QŒ?îy(é`à?Ÿ^/ªuR?¯xmpŽ?Ÿ^/ªuR?ïv­˜þ?qóü£¥ð?'*M—C©?qóü£¥ð?î¬yºDùž?¢)É!"¿?¥8d^D?¢)É!"¿?ì¨Ï9'?Á.Fˆê8²?¿
¹†7ÖË?Á.Fˆê8²?éë'ö"x˜?°¥xÐbµ?ÈQ¸%î¢?°¥xÐbµ?ë'ëôQÃd?©Õ^Q%(Ý?Ã`P.¸òr?©Õ^Q%(ÝAGN4FGL J1959.1-4247?àZÿ™ÂxÀ>ÚQÎÀ9]X «À<ä«ã£@÷8 ؽœ@(V£zÃë?µPNÅ_ñ?ŹH
°³@
Ár%·@ÆÈo(¿µVçÃH>³¿ÜMÍ=`Ó¿åªåò7Àa¿åÖmàXDæ¿ïS_²¿ïù7Y2¡=AGNfsrq3FGL J1959.1-4245PMN J1959-4246?ïö¢ùê'0?YH"qãq?Rºu0i?YH"qãq?ïõu¨×,Ö?WÒx€ãž?U®jc"Š?WÒx€ãž?ïPµçò>?Œšµ}™Á"?•éCZNP?Œšµ}™Á"?ïÿ™ÏZ¬Û>úS=ùџ?	Œ#0rµ>úS=ùџ?ïô–Ž]Œ‰?X""y­?VÒâõ/ý×?X""y­?ïÛO@§\r?yörÏoV?rX_'4¿?yörÏoV?îܘ
½? Ÿ …ü@É?¯OÒ5£m0? Ÿ …ü@É?ïÿN
5I?ܵ´ %?Eyŀ®?ܵ´ %AGN4FGL J1959.7-4725?ïîÆÁ½F"À>Ø},{‰
À9!´:.Ï÷À;¿"(fQ@S±uƒdÏ?ù{üä?®Õ¼þ ?ÀqW†#Æ@À­Ù©@ö"Åš)¿Û¾P§ET?ñ³6#¿ÔÊ¿ÁÌh¤¿Ðï»dD£¿ß†—D¿ã|}`þÈAGNbll3FGL J1959.8-47251RXS J195945.8-472531?ï¸áÔ¬ü3?€Á%§ióÝ?ÇŠÔhý6?€Á%§ióÝ?îÒX
Cq?¸õg,¬RÑ?®'ÚƒwKï?¸õg,¬RÑ?î=ŠÁ~SÝ?žÕ™±Ïq?¬'Sèö©3?žÕ™±Ïq?îî}|‹Š?†Ž¤Ç?Ý?¡(;™šW?†Ž¤Ç?Ý?íÏ,ºŒó?±–c¼wpù?±†š+˜gÉ?±–c¼wpù?çE±á¹^?Ð{kBG?Ñtœ=ҍE?Ð{kBG?î"üÍ#<y?žÔk%¹l?¦À3-Ì8u?žÔk%¹l?éþ3¶3?°úÙy?È1&‹4?°úÙyAGN4FGL J2000.0+4214¿á.ÇÌÿ#@ÉéÍ³}À:-ÏZsÀ;¨ÕÑXLÈ@îd¥q>@]_V§­?Ãà™~욿 ]æ»?ÜŠ]ÜT@eLÚÏ¿ä×MÄ®ñ¿çûÃà•®¿èKÈö~vþ¿ä-RòK¿æ‹È ˜;v¿ïC¬ýúlAGNbcu3FGL J2000.1+4212MG4 J195957+4213?ïþ¨s"»?"^èk¾ð?/…wãŠñ?"^èk¾ð?ïðˆ´wžü?eãæ°åk?^î—B¨ð?eãæ°åk?ïéëÍTB^?güA]±?f2‰aŠ?güA]±?ïÿ5߶?4¿'í?yVòÄÇß?4¿'í?ïý ~Çþ~?3†HñuªW?6ü	zÇ!'?3†HñuªW?ïqà:? lîk³ a?'Ãü/[n? lîk³ a?ï´Ù0]jê?…	>Z?'ɳìl×o?…	>Z?ïûú—¤?4³—¢ g•?@¾	7ã?4³—¢ g•AGN4FGL J2000.0+6508¿êŒ:
'Ö@1ªDØw$ûÀ6ï.¾YlƒÀ:é">¿@¸L]{±&?ü.ˆ>''ü?mJ—do?›°]ÓùE@Ô>š4@*æ';Ù?È˜=V«¿Ó¬%Ã'í¿ÚÄLÉÝ.¿Ùt-݈ݿà¯ÁÏÖ¿Ó_\òI^AGNbll3FGL J2000.0+65091ES 1959+650?ïý"zVïa?1â]´l0?3d,Ýkf?1â]´l0?ïòò¬ÁzÅ?`yÁ­¡ó·?Z¦ø¼d¬?`yÁ­¡ó·?ïÁÕ?…â øÇG??1s²U°g?…â øÇG??ïÿÜ)i¹`>ðôýroJ>ñëHu7¿º>ðôýroJ?ïúۙÕdÝ?Dp½g(é?D'˜SI?Dp½g(é?ïÁð?ŠXŸI?tüôXE?ŠXŸI?ïӏ|½ÉW?*ìKòä?v8A¾§ø,?*ìKòä?ïÿîîñËñ>ðØîõu8>áÐZ+Â>ðØîõu8AGN4FGL J2000.3-2930?çILWÏþÀ:þó¡LìBÀ9x>£©½ÔÀ;ýû›ût@>Kw1@‡ª4ò?²+g¯fµ?ªž,a™`?ôYè'u¹?øh5Uø/&¿ÙíÚ£úñx¿áf½+-«¿æª°þ:-"¿æ|ZYê
¿èþ»ýq°G¿Þ	5]ÚѝAGNfsrq3FGL J2000.4-2926PMN J2000-2931?ïáO@—?hlÜLêÖ?ní°Ò°8…?hlÜLêÖ?ï3ƒ§ƒ¬?«fœJ±¦—?™ŸÏ‡Ÿî‰?«fœJ±¦—?îð
\ò—?–J/'!­? ÿ] r?–J/'!­?îAƒµy?" 
,A?«çĦ¶Ù3?" 
,A?îßÿTçì?ž9?fÈ6?¢h8?ž9?fÈ6?éPüÿ'èm?ɘɽI¥?'¸^M?ɘɽI¥?íŽh&cË?¢²¦‰UÏv?³Œ»ø"¯©?¢²¦‰UÏv?åIQW¶uG?º%¯Z(É?Õm]P"q?º%¯Z(ÉAGN4FGL J2000.6-1328¿ïÿeÙ§ÀÀ5QÇ5ï¦À9Ãí~<QÀ;ý}K…9@ø‡Ô3@ÝS¨Á?·»júŸÃÕ?µ=ä7
?ùš£Ÿ¬Ù@ózÜÀ
¿Õ·"ÁÄO¿à®È4·—±¿è (ÿӊV¿èÓ}æOU¿Üöÿ<
È¿è<ýâC'AGNfsrqTXS 1957-135?ïþ~y¾Ä?$™|~¤Î?/8e¼;h?$™|~¤Î?ïß8·×rB?v…`:G
–?pc¤
§öï?v…`:G
–?ï陜Ò;Õ?f
ÙÜ*'?ffcCÁªÁ?f
ÙÜ*'?ïð÷¸Dá?Cåölɤ?^ëSX?Cåölɤ?ïû#5Óæ5?CÀð.[Nä?Cs([0ÚÁ?CÀð.[Nä?ïM.IÇý¹?›Ý0r8­?–Z6Í߀à?›Ý0r8­?﫲 Q?…î¡ÝM?…>¼E™{â?…î¡ÝM?ï™]»‹Ë•?vgƒ§~Ü?‰¨'~ä?vgƒ§~ÜAGN4FGL J2000.9-1748?۞QêƒlÀ7çF˖lÀ8®Í"]"À;˶…ì>@Äm/ƒPW@
4†ðIª?¤®ª¢ÖY>?½[¦Õþ`?÷jÈ˶LX@P¨dÅ?ïÁcâþ¿àØÙ`ð¿åú%Ëk£½¿á4&­é²·¿èy4j¤9¿Öð-¤þ҃AGNfsrq3FGL J2001.0-1750PKS 1958-179?ïúøÕäÎ?t|ð-?DFÁ+²?t|ð-?ïçCÑ;Š?pÇX=#?h¼.Ô½÷?pÇX=#?ïâ%°ØiR?s#.ÇSg6?mÚO^mÇ?s#.ÇSg6?ïú÷^Š"±?6=GY'q?D""ՁR?6=GY'q?ïöÖFÚ@9?PߑýÎ?RSr‡ø­‰?PߑýÎ?ïnQßƤ•?œ7aŠkh?'5Ä
¥c?œ7aŠkh?ᄂÁÁ?ƒ
TIe¤?€~9¤ÿ¸?ƒ
TIe¤?ïø0<d?DOŽ­'¼?O?†]›|&?DOŽ­'¼AGN4FGL J2001.2+4353¿ë—ô™Ö'ƒ@t3ÿ
zÀ8É16Ù±À;7ì]‹ÌQ@‹7Ö[û?üùä"rÁ?¢¼'Ÿ<ø?¸ÄP@N¡@«â´•žb@"7Ð%¿Ýù7Ēk¨¿ÚRðÛö¿Ö2ü´›þ¿Û!ŠßlŒ›¿â¸oG¶¿áö˜ã'4pAGNbll3FGL J2001.1+4352MG4 J200112+4352?ïÍ4ó•†?±L"'à1?ye¹5=?±L"'à1?ïÝ»³†?{¸®e¹,Y?q"&E7
d?{¸®e¹,Y?ïʘ¿voj?'J‹'c{?z³ Pvö¼?'J‹'c{?ïÿ¢'KtH>ý¡ý²Òž?_tÏüœ>ý¡ý²Òž?ïüKüœ?4×ÌÖJé?;… V{=þ?4×ÌÖJé?ï/÷-bS?­ÑNcÙù?ŸzSµ¬?­ÑNcÙù?ïÎz˜¼=Í?‡bA";š?x³‹ã™‡?‡bA";š?ïÿxŽº¡?	ã3,&?î%¬Ú"?	ã3,&AGN4FGL J2001.5-0818¿×i~–*p¹À3TFù¹"âÀ:Ш·CΌÀ<B
Ìsá@žŸä@OÒ}浬?Ä2"ý[
¿™f`ݐ?ىVá
K˜@Àû*XC8?äzfކ]¨¿å®‰J–ý¿ä{Ëóˆù8¿âÀ_C‡i¿Øyx;ûÙ«¿Ûƒ½D³«AGNbcuPMN J2001-0820?ï»É†Áj?µ&h›0-Ö?
¾¦Žµ"?µ&h›0-Ö?ïç;£ø Ä?qB,"?hÄ\Ý\1?qB,"?ïòhcP¡?g¬ü¾ãC?[/ùhm‡?g¬ü¾ãC?ïýܞ?àZ?"ÛŸ¹¾Ë?1áԐ1?"ÛŸ¹¾Ë?ïý3f¬(à?8uqÉ'?6dËýw†ƒ?8uqÉ'?ïQ5¾£?žæ1ŸJ¸ª?•Ù^î‡cŠ?žæ1ŸJ¸ª?ïïÈÙ^fÏ?qO¨á¸#?`7&ÈÐø?qO¨á¸#?ï÷¯NÙ?C›{F
×]?QÄ¡p'½î?C›{F
×]AGN4FGL J2001.7+7040¿íûœyP€@3õXÙµé[À:Ÿð˯–À<Mҍ.#@ùX…Ó8@ó:G#«?¸F	¤™|é?¯ãʝÑc?öGŬGH@.çÉþ;?×¼ÙûŸa¿È
‰*‹™Ò¿á7'Ô'½¿âa‡"à¿á`žü/¿çŒ:€¯gâAGNbll3FGL J2001.8+7041TXS 2001+705?ïüÖñ"9?(.³I~†?9Hwt»`$?(.³I~†?ïîÊ¥?bKpé炸?a5õ9»S!?bKpé炸?ïõݚØçk?SÅ\»¥-?TDÊvzt?SÅ\»¥-?ïӌ8ÕV?W	{‹03?v9ã‹,5?W	{‹03?ïòÞç¬w?RóøåvhD?ZB0öÈÁÌ?RóøåvhD?ï´
LpW<?†ã»ßfBÚ?'ýlßʨø?†ã»ßfBÚ?ïñ…c°?kXö–Ïc?]Üõzõ t?kXö–Ïc?ïQ´Ak	?zçˆß'ð.?•ÉwÕ:Ù?zçˆß'ð.AGN4FGL J2001.9-5737?ê-/|ߎÀ?÷ë[-M@À:‹¹ÝÀ<Œà«¦âW@ðDK3…?ÿÙGÏ¢j#?Á·vÙ%K?¶W´ü?öB;C¢ìÿ?ñ>¹Ôw'?ïùPMö-¿Ô]Oö¸Y¿åP
nîË$¿×[l7`¿]¿Ûû+ÚÏCõ¿ïÿÿÊPËAGNbcu1RXS J200205.7-573644?ï÷-Ñýì³?UWÇãì"?Q¤[£ñŠ'?UWÇãì"?ïˆ!â}ä?—'½tšO°?÷‡Y§Æk?—'½tšO°?ï³÷
""?"¨§BÀj?ƒ<ž«w?"¨§BÀj?ïqçø2'`?v9¦G-@?'Ãô†J?v9¦G-@?ïìæðåZã?kŠ/?Dû¾?c4Â$¶?kŠ/?Dû¾?î1ØSŸ?µK.+haß?¬â~·Vs?µK.+haß?ïŸaè…îu?ˆ E¹W?ˆ'…Þ"bÙ?ˆ E¹W?ì¬+×õû?¡{àÆàÂ?ºž¡@W%?¡{àÆàÂAGN4FGL J2002.4-7119¿ï"Té'À?@®û*®)À:Ë«®o´À<'°P$Ü@!ªñ§L‹?ùèäZˆ?Äþ2J€ì?¼"Ôeh±?÷r¦É¢@#'+f5?ïÿÁìžú,¿îÆŽÜ&?ÞSÇÝúœ"¿È1q'"[¿Üƈåí/C¿ÏpÜÔ+çAGNbcuSUMSS J200227-711940?ïþˆCa?ôŸU]´ý?'wë¸P|}?ôŸU]´ý?ïôT÷ºGu?\+ÜQ a?WV-ûµö?\+ÜQ a?ïñ	®Br?f`±©°?]ì£{HŒh?f`±©°?ïóؙ"•?CZªÈ½ÐG?XNÍO¡ü[?CZªÈ½ÐG?ïþ¼¼'ô½?Nž©ùr¶?$45Qº?Nž©ùr¶?ïØÕA™(?xÈßÀ5ö?s•_°xH?xÈßÀ5ö?ïôZl÷¿?e2¸3?WK¯€á'?e2¸3?ïæQ¡;;?^N疕á?i®^ðùÄQ?^N疕áAGN4FGL J2002.6+6302¿×"öÃp@0q€²BÀ;qPþU0À<Ô®¥šXÜ@""¸;›6¨?÷¤G¨5=Ï?Ðg¼'c?ÐWˆ
€@=Óºý—p?÷ÙÙò$J¿í4DÀ¤Jx¿ïÿê o·?ð¿Ç—…BI¦'¿ÛåœFó¿ozFm!ÁAGNbll3FGL J2002.7+63031RXS J200245.4+630226?ïûs‰±õ?9¨"Á†•›?B1ÚùB'=?9¨"Á†•›?ﴖUþux?Žï6)æ?'ÚjŠŠ?Žï6)æ?ïēü)d[?w‡ÑŠ" Ž?}¶«*b?w‡ÑŠ" Ž?ïgWöi±Ó?€c[´vâ?"+ꍪ?€c[´vâ?ïûƒ ±Pp?;H[pzë?Aó|7ÎæŠ?;H[pzë?©ã"¹?µ|4@êÏï?¥ÅÕe6`p?µ|4@êÏï?ï±miÿ'à?…iEP݌9?ƒ¤¥‰ºoý?…iEP݌9?í‹Ê<sE?¦ÎK}'?³¡¯øLÕ?¦ÎK}'AGN4FGL J2005.1+7003¿æ+`Ío@3oÚè'®À9ðhÒQqÀ<#ñLÞÕä@ z¾©HŽ9?ú;o&ÿHJ?ºÀˌ°Ó?Å®6Jü@ÍÀ:S@ð6¿ãXò?Mé¿ÃþFïƒÜ¿ÑÂQž®+w¿Ð:² {¿ßGC…:è¿ä¢ Æ´…AGNbll3FGL J2004.8+70031RXS J200504.0+700445?ïúAêR'?B!w´†ç?FøWNùX?B!w´†ç?ïì•tÆÑ`?h–9jdå?cj‹3¯?Ø?h–9jdå?ïÙüÂw£?t¾~ªþº?sžÓüª(?t¾~ªþº?ïìêhábR?E7DQÈ.?c—*üEr?E7DQÈ.?ïòÀ{Ó'?Vs'M¼Í®?Z\¼ŒÂ?Vs'M¼Í®?ïx÷ɶÔ?žZz7
9M?‹áÂPºï?žZz7
9M?ïygûÅfZ?ŒiΏjwµ?Óê:¾?ŒiΏjwµ?ï¼kû¢"?l*¦åæ?€å8«9?l*¦åæAGN4FGL J2005.2-1822?Ô#šyðÃÀ8Gà·õ¥À:YEnŸÀ<o㽪@´"¢lQ@ÜòB9`?À¡âhjx?0°[@+kÇú*(¿ÛŸ¯È°š¿çèµ`Ÿ}¿ê@bUµ"¿â
r_C¿îØð²È?çý/Á
ÑÐAGNfsrqPKS 2002-185?ïúfÜ`œ+?@€ÝñÇ\è?FdŽYÓe­?@€ÝñÇ\è?ïé©Æ|?…?q/»\G‹¨?fV9ºº:I?q/»\G‹¨?ï­ê)æ¬?'³Fò`bÊ?"…uZLü?'³Fò`bÊ?ïüæ%?-ù/—Jq'??ïºÞ›Õ×?-ù/—Jq'?ïî³#OÝ°?b{Çù–?aLܗeá?b{Çù–?ëgd?—­HŽiXÂ?ùœ•Âù?—­HŽiXÂ?悔åd"u?ˆÉö§¾TÍ?…І™ rÈ?ˆÉö§¾TÍ?ïèd¬Á®O?^…
.?Î?g›SgO?^…
.?ÎAGN4FGL J2005.5+7752¿ëÛ¿*2Œ@6»½¯ljÀ8cSÒåë'À;ºåaïa@>®ïl4@"]ªÖ?œãàBSX?ª[<D\"@
ßE™›@¿ž$DÙ¿ÅN	¸»rÝ¿à'úáˆÁ¿ã¼Lßx÷¿á{¸<òϖ¿æÄÕA»a@¿åA".ÎI¥AGNbll3FGL J2005.2+7752S5 2007+77?ïýèmèô?$~µ¼¿?0¼'7 ?$~µ¼¿?ïô¥_å1·?XÕ´þ&‹?Vµ?Ò§Ññ?XÕ´þ&‹?ïïñ Ii´?X~¡¼—ç8?`_œŒK?X~¡¼—ç8?ïþ'nEò—?ÏLG$'ý?&Ù"óíã?ÏLG$'ý?ïþ%œ
¦ç?!îjþŠ?-¦>¡œ?!îjþŠ?ïÿOYž?…ßފK?~ ~jáÃ?…ßފK?ï섫©o-?qVLO®9?c{T™é*f?qVLO®9?ïýX|ùë?.Á‰"5S(?5;…îÇö7?.Á‰"5S(AGN4FGL J2005.8+6424¿ï8L
Zíž@0Å:æ…ÛwÀ:f™5ƋjÀ<7w^@1a¼­ž@†ö¼Š_j?Á%x	¦ó?ÏWá&öå@b[T‹@Ձ†R?ïòJ¶Ýw¿ÌÞXeqÉÇ¿åêûVM¯¿ãG¦¢–˜]¿ëÔ@ßn:¿ïùö€û=#AGNfsrq87GB 200541.3+641601?ïÀSЕ6ç?xW`J«½c?Ö»"Øz?xW`J«½c?ïâd—¡?q:rւ÷J?m›€mÞ]Î?q:rւ÷J?ïLƒ"b‡?Šù@}†"?–ok(©(?Šù@}†"?ïÂC#›?`®r¥T.÷?~À^‹êB?`®r¥T.÷?ïÖ§þŒ?™À0xÂ?Ÿ…*þ" {?™À0xÂ?ïoºì¡¡?š.Þ¸þ%ð?'¼Daî?š.Þ¸þ%ð?ëü"[°¼?ªêH(z×é?Àv'=ç?ªêH(z×é?î‡åÝÈ{7?àú†bgü?§¢&çè‹?àú†bgüAGN4FGL J2005.9-2309?ïžØE%ùåÀ:#'ˆÀ9 Á¶UaÀ;Þ{ÍÖ¸@HñS¿Å¨@19ÓÀÝ?¯XËH=[€?¹"IV
N@<êy…ýÛ@b¥ç…µ·¿ÕÅqú_r¿á.›‰]â3¿æô÷ŽAvÿçÌ.¬­¿æm¸¸ÇÝ¿ïÿülòAGNfsrq3FGL J2006.0-2311TXS 2002-233?ïþâr?$ßùÁ©‹8?.àZ=ob?$ßùÁ©‹8?ïäo°‰l?yÀ¿ÀÐ5Q?kO¸‹âv?yÀ¿ÀÐ5Q?ïÝõzžŠ?q#*˜U/?q{….ö?q#*˜U/?ïÿYT¸œ?`+ë«ì?Õp${3?`+ë«ì?ïþ)`ÿþ?!•©Ÿ÷Ó?&ým€˜`?!•©Ÿ÷Ó?ïXæsƒ?¥JgĬ°?"ý/ç!­?¥JgĬ°?ï¢S[¿í?‡8–•hh?‡k)ŠØ§?‡8–•hh?ïþ'#?9rÅà?&íÍÉËv¶?9rÅàAGN4FGL J2007.2-1433¿íê›÷³"À79~ºñ6À:TÌ4 ˜ýÀ<'¬-ðÔ@åÅj­É@¦rÅð9¹?̍ÒfÛ)?è% }ä\`@lûï¯P?ûœNOnRC¿à
sáÏw¿Ýe~_–~¿æÁ³"¢Ú¿ï¹û8ðâ¿ËÁßeUÅ¿ïÿþBe«+AGNbcuNVSS J200711-143205?âÿ³'Fǘ?Ð*ÁO;ü?Ú˜ÛrpÐ?Ð*ÁO;ü?Ðëª[f`»?ÊJœ9e?çŠ*ÒLÏ£?ÊJœ9e?åHÈNôëá?²êT±­îƒ?Õnob(>?²êT±­îƒ?à5ý"" ¨?À$dp9p[?ߔÖö¾°?À$dp9p[?ÓB'¾«nP?ÏZuä«M?æ^¶ ªHØ?ÏZuä«M? êý°nÅ?°-	ë&¯5?îñP.ÿT?°-	ë&¯5?ØÑgÿÌ1$?ÀŒe²m?ã—Lçn?ÀŒe²m?˜t"Òíí?›DÄíÈ?ï<^éM¸?›DÄíÈMIXED4FGL J2007.2+6607?Ó]H¥¶2'@1s›fù3]À9Ò"ÿ‰;À;ñgº#|Ý@¢
¢Ed¹@]e¼{a?¿2ŸÝoK?÷9½ï§@'¬'\f@lÐ"l¼l?²2³=ځ¿çòêmDŽ¿èÖÁ½Ð»¿è7çÍÚ¿ð?ïÿþR€ÖTAGNfsrq3FGL J2007.3+6605TXS 2007+659?ïÑÖ-ëíò?­µÚ¤•?wèñûÃK?­µÚ¤•?ïð|¬+©?e\a¤ù?_àé¡.7?e\a¤ù?ï¡Ë+`'?…F"lãbx?‡9x—ws?…F"lãbx?ï÷ä1î:??è'ÄØÓC?QÊ79.Í+??è'ÄØÓC?ïà›ÍÀ+˜?s|8~¯Z?od2w¹?s|8~¯Z?åápÉ?•+›E]…¬?‡F•b=½?•+›E]…¬?î'k‡/@?œ3"Â?¦ÙG'[~ù?œ3"Â?ï½9P'Ë?pþž§… ?€±«õûN?pþž§… AGN4FGL J2007.3-7728¿êhSjOÀ>†yF<û3À:k‹dL°³À<G¥«ö"p@.ß/ûÆ@F5~g?ÄxH:	ç?×±0@KA¿½ð'@¨žÑç¾Á?ï¿5¾§¿Ù€_ víó¿âûH
ZÍ¿èÙéëÁ"š¿ïþâßâÍ?¯aT¿Ü	½AGNbcu3FGL J2007.7-7728PKS 2000-776?ïE8•Œˆ~?•€)Fz´?—XíUN(<?•€)Fz´?ïñå¬5[?_ˆä+jgT?\5ú™ÖÙ«?_ˆä+jgT?ìâ÷]¼k"?£;˶‹è?¸èEøí?£;˶‹è?ïôŒ×ê7?B.éíf8?Vz旣q?B.éíf8?îâÀK€?¦ª‡Ã!`?¡ÓûDxbº?¦ª‡Ã!`?ïÕq¾Åg?€&Óíh#Ü?uG}¤è…?€&Óíh#Ü?åLÛÐË´õ?·%ÁX~?ÕfH^h–?·%ÁX~?ïÅÏ)ôE7?j,C·é?}k°—?j,C·éAGN4FGL J2007.9-4432¿í´Eñ•ÐÀ?ؖþ´¦eÀ9tÓäCÀ<€§ZL}@k›@½Òtw?³–Ç'5#ù?ÀÖ­ _@%çñ@ccK©Ì˜¿Ù/-••¿ã™*]÷'¿çèÎUcä¿ë¼[ed¿æŠX^©¿ïÿÉC«P{AGNnlsy13FGL J2007.8-4429PKS 2004-447?ïþã‹ç:?/}­BϛÊ?!ÇE•à£V?/}­BϛÊ?ïôM1£Á?d1Aµ/Œ?Wež1²>Q?d1Aµ/Œ?ïŽe3?€Š¢:9þ"?~>¸ÀWöÅ?€Š¢:9þ"?ïþÌR×?†)¡xY?."@ɇ:?†)¡xY?ïÿ}9DLê?¼8
R ?XՄVú?¼8
R ?ïÒՊW?"–é+T?v•;ø<?"–é+T?°ôe?ˆì\þµ'?š=SJ°?ˆì\þµ'?ï÷^lÈ?Gâfs'b?Qõá	m§?Gâfs'bAGN4FGL J2009.4-4849?·ú5'…XÀ@M!…Æ~À8.C~ÚÑrÀ;g1Ԏb.@pÁñÒk?ûü݆Xt5?ŸÌØؖ&?¤"^$Bú@é%»{k±@(ýâPm?×¹ø^ËèK¿Ö€A#5å¿ÚÑMD×J¿Øj¦sG¿á·zö@c¿Ð‡á@!X?AGNBLL3FGL J2009.3-4849PKS 2005-489?ïöŒ`˜h?"kéëf?Rç>¨³C3?"kéëf?ïôI®ÓE@?k¡ ·º¨È?Wl¢Õ'pO?k¡ ·º¨È?ïÚWãÓ?µ×'ÎyJ?rÔvèr3?µ×'ÎyJ?ïÿFtâÐ?¡[¥Ó?1k¢*¤<?¡[¥Ó?ïÿ|²zˆ?Êc­q¼?pfõdÚZ?Êc­q¼?ïÕ@;.n?‰ÖM"I`?u_òæˆPï?‰ÖM"I`?ïÞi é«;?y/»¡ #?pË/w쒑?y/»¡ #?ïÿ&B}u?œE'\ª?<W¹ÿ?œE'\ªAGN4FGL J2009.9+3544¿æTáž'W?õÀ—Ì:À9«ð©JèÀ;8&1Âð«@ 'ã'ØD@‰éÍ³}?ÑBDþ·«}?ºëÖÂæ˜?ëȆ·>Æ@	eˆšî®?ïÜyGêz]?䪯k"¿æäMÝX‹1¿Ûì{ÿ)ì8¿çgš®lu¿ãÙÎ"7bmAGNbcuB2 2008+35?ïý€4~óâ?7OhQ 9•?3þZÄн?7OhQ 9•?ïÐzì&ѝ?†y€JÄ?w‰ÿÕ4?†y€JÄ?ïÅNFña?>ädÁ'0?}Xܞ$»p?>ädÁ'0?ïÌWÆÝÁß?bE&ÌܵÎ?yÔŒÿˆ†?bE&ÌܵÎ?ïü2Ò4?A&˜©º?>oñ2¤c?A&˜©º?î˜1Œao(?³4:hË_S?¦|ç>4x?³4:hË_S?ï[2D–?—«ø¢Û»?™·n
F?—«ø¢Û»?ïDžð=Æ?ˆÅ=®®¡?—l!ö¦¹2?ˆÅ=®®¡AGN4FGL J2010.0+0726?Êß9¦®šÀ+}|o½'=À:"ãY×À;Ô¨ÒÁ'@7ŽÆÞ@M˜¤§Ö?ѓ Ì"Â?Ì5¾=gêu?ùZÔG'‡@Ë-´™$T¿ïÿH è?ïòøp¶L¿æðf…p¿é$©'¬¿ïÿëþ@bF?ä"Ä?µwœAGNfsrqTXS 2007+073?ïŽeíUê~?«®ìzÝ®×?Œf"¸CÐP?«®ìzÝ®×?ï7—x?¨ ­÷(þÂ?Y
ÑÄ'?¨ ­÷(þÂ?îo$U"?—Ïø!û'Œ?©
¸
B˼?—Ïø!û'Œ?ïYåÁ‡Á¢?~aµê—"Û?"ÃGÔ/5°?~aµê—"Û?î2Ñ?­?¯ÂZçƒç"?¬ÒìRì3?¯ÂZçƒç"?æF=&&/?Ñ@%g¡,"?Óïs…³³¡?Ñ@%g¡,"?çÄ1…‰j?³l>H1ÿ?ÐwœôíÓ-?³l>H1ÿ?è ¶·jB?º•æò´?Ï}%"VõŽ?º•æò´AGN4FGL J2010.0+7229?¾',Zz@4*Öý¨6ëÀ8Ö§i¦À;пB Ž€@œÞ¬ôd@•ƒb¯É?¥f¦R9³«?º‡[>7Å@Ñ2^!‡@Oø0Ó²o¿Ã¶¨@οâƾ?ì)4¿ã<î
ö¿ä'õÉEY¿ç£S¿šµ¿ìcÝ ÁAGNbll3FGL J2010.3+72284C +72.28?ïûû»€R??˜]øFõX?Cô°D6??˜]øFõX?ïÞ
(ð0¡?z¾Ãm%8ô?púënz"c?z¾Ãm%8ô?ïÚ1ˆIvR?yÙÃÈo¯‹?rç;â$
?yÙÃÈo¯‹?ïÃPåÔ8Z?`aO"ú'ë?~W/Pï?`aO"ú'ë?ïúÂW93?E—Fò‹?Dö¢÷wÙs?E—Fò‹?ïo¿M'?Ÿ-CS=Ÿ?'h&¿?Ÿ-CS=Ÿ?ï7üä?"lŽôzæ?œóà?"lŽôzæ?î'ÄF|¢N?ØÑUf?¦Ó»•¢&!?ØÑUfAGN4FGL J2011.6-1546¿Ûî²PÛËÔÀ8°0ã͚RÀ:vJßø#À;Ю2­Ò@ûÒBØl¾@–ž<–‰?΅ ¨×z%?Õkã=|D@²fŸqIï@é^‹P«"?ìÓÀ§$œ—¿æ"Ÿè¿é­Á±ç¿íŒQGpÅ¿ïÿñò÷¿àšÓá*ÕAGNfsrqPKS 2008-159?ïÊÈnÕ[ù?‡ƒµOÚ=6?z›È–ï¤?‡ƒµOÚ=6?ïB´ŸHI?¦­^³Ä²?×©q>`Ø?¦­^³Ä²?î_¼Î}ç?œYhCcÁ–?ª3 «Ö?œYhCcÁ–?î›ÇÔý²?…íSRؽ?¦C'¼¬oê?…íSRؽ?î·%?"B³›ÝÈq?ŠØNÉZµ?"B³›ÝÈq?åš}ôïÍû?Îw•]?ÔË d
?Îw•]?ì
›rj^K?ªn%ÔNA?¿«$l­
¦?ªn%ÔNA?âè®»ÐâA?³suÙÑ.?Ú.¢ˆ^;}?³suÙÑ.AGN4FGL J2012.0+4629?éÅ.Ê\žÖ@sò«´NÀ7ùvjNRÀ;+ü™C3@щ³¢?þÌÀmBùz?¡ð}^®Ø?¹DŸÂ'­C@±þë-@°fŒQ®?î~Ó-A¿ÙI‰`çK~¿Ý%=ð%—¿ÝæúÀ¥÷÷¿å2Hø"¿â!Ý Y§AGNbll3FGL J2012.0+46297C 2010+4619?ï÷'P8ÁV?P¾S"|ü6?PÝ_DEÛ?P¾S"|ü6?ïÔö©á?ƒ´Ý+×?u"«mýï?ƒ´Ý+×?ï¿Î:%?ƒ¡Ñ– ò?€'¨¤—?ƒ¡Ñ– ò?ïøõùے|?<ñkŸhP¶?L(ÆÙí?<ñkŸhP¶?ïûOû|ï?:<‹6 »ì?BÀ–	HJ?:<‹6 »ì?îæ~±zr?¬ƒ/åißi?¡˜4qß?¬ƒ/åißi?ïÊ&a5?†}Èúý"?zìÏ]3)~?†}Èúý"?ïð:¡ÖBÜ?TªosaÞ?_Š¼a8·Ô?TªosaÞAGN4FGL J2012.2-1646?Þ¦çô#0À96½ÂmÎ:À9‹¨"ÉX¤À;DŽŒÂÂ@ê¾¥AÃ@¯ï¤h)µ?¼Ì8A(Ù?Øàc¢¼­ñ@³}pn'@	˜JA¿Ç¡QHòã¿ágºú<q ¿éÖæ+B¤¿ìKâV¡Í¿ïÿs+(x¿ï`,Æ1¨AGNbll3FGL J2012.1-1643PMN J2012-1646?îG0—2È:?±èßc8›?«Œö¯cW?±èßc8›?îÀI¿š<à?©ÚB}i?£ûd¯?©ÚB}i?é¦[ãš]?°"¼JáŠ%?Ëåfq–Š?°"¼JáŠ%?îí¿è|št?ˆ_%OPèS?¡$y?½?ˆ_%OPèS?î¡ååÄã?·aÞlÊh?¯õá£[Ò?·aÞlÊh?å4°++|Û?Ï×J\ÎÔ?ՖŸ©©I?Ï×J\ÎÔ?ê6ڜ'U?­øÊÿ¯&?Ç$•½º®?­øÊÿ¯&?ãgÆLCê)?¹ú
Åý?Ù0sgx+­?¹ú
ÅýAGN4FGL J2013.0-3717¿åÇF½Ý#À?‹UX!)EÀ:…Þ\AIvÀ<OÄøÂôÝ@'T-©±@ØIёX?Å6>5è?·æ4|ßN°?ï/_¿_@%;Qå¥â?ï÷5¡L–\¿à—¿9fS¿åÜ=ƒMÕ¿çUr¼Å¿è
g'E?$¿ïüÁr%·AGNbcuAT20G J201248-371941?ˆT³ó?µ,•:Ëi1?Š]õ!×K?µ,•:Ëi1?ïÑ֗%öà?ƒÆ:Êöů?w´S—tV?ƒÆ:Êöů?ïJFà±?•Òl¿ˆü?–·#ÿIÝÖ?•Òl¿ˆü?ïÎð|W?^9µõÅ{?x‡÷ÉcUw?^9µõÅ{?ïÚ½Ñ1`u?y#ú¬"(-?r¡]ñs?y#ú¬"(-?î˖'š?¬ìfôjpm?£FŸŠjÔ?¬ìfôjpm?V‰O?ž]‹ú´6Š?¤Wj˜KÒ?ž]‹ú´6Š?ï§k¥{¶?"]>=á?œ†)??"]>=áAGN4FGL J2014.3-0047¿ÙíXð©mDÀ2¿õÆÁÀ9ñÎWçG¢À<l­¨DW@ >eû²hs?ÿ\ÝP¨?¹›ý¢È?™µ ü"?ãcÓCßRá@
±ÇP·?ﶿ¹Sž¿á¦Ç…ò¿à7@=ݱ!¿Ú1Å{`¿æmP›#•¿Ô'xŸ£ô¼AGNbll3FGL J2014.3-0047PMN J2014-0047?ïþC|Mû®?!Wa¨…?+È>ýԝ?!Wa¨…?ïß²¹aqE?ߜw`Yë?p&£b…->?ߜw`Yë?ïó3åú_?^€b´Vê?Y˜49Þ?^€b´Vê?ïôu+ahâ?B!KÖ?W©ÃÞë¡?B!KÖ?ïü-ší׉?6wáÕN®?>")•ÙF?6wáÕN®?ï>\õ¬óq?¥¶C2)©å?˜4aL_Ø?¥¶C2)©å?ïß¾©Öu?wÙ¸C®ûˆ?p ñÖõ"?wÙ¸C®ûˆ?ïèBÖá›?Tòñ?A
A?g½)B èT?Tòñ?A
AAGN4FGL J2014.5+0648?͘xUëÞ¥À.ï»À:
†¢F†À<MÝÙd‹@!/òù²3?üæÑáÃô?¼"À^ÕMz?¥~ü¤¿?íÀSí"?üÑPÒÖQ0?äÔÀ¡›EÁ?|jâ"pv¿ÕN\¤›«B¿Û'oü'7P¿Ø<EÀÿd$¿Ü‡5^0·ÙAGNbll3FGL J2014.5+0648NVSS J201431+064849?ï÷¢Å¬
ú?Gyc_ÿÙl?Pºtµ¨{±?Gyc_ÿÙl?ï¿{RS+n?ƒÕ"šzå?€!+d­â¥?ƒÕ"šzå?ïÚ©Š¹"?q@–@ô9í?r«:£æ^Ï?q@–@ô9í?Õ˜?r¨w¶x€"?ÐJÀ'Ü?r¨w¶x€"?ï۝X§J?mçw6-?r1SÉN'³?mçw6-?îU8Çû4?³g×¾Ñ1?ª¯Üu8·?³g×¾Ñ1?ï°]Kƹ?…+ì/–?ƒè­Q¸–?…+ì/–?îI¯åœ¦?'ƒ)'¿¿F?«e¦7% ?'ƒ)'¿¿FAGN4FGL J2015.0+1621?æS¿J¶»À$L'ÿK¥À:{gkÀ<™%ÖS^@7Ã¥†·À@!Ì{n5h?·?äq"&Á¿˜Ýèº$dÊ?ã K.Ò{b@5O&óû?ïÿíöé	¿ænyÖ]¿åjŸb0w¿ågÕÒ/]¿Þڌ}ý0Š7{í6OAGNbcu3FGL J2014.9+16234C +16.67?ïî,«¯›º?gÔkCœ?B?aÓTt 6J?gÔkCœ?B?ïÔC¡jsf?'†¯›ÈK?uÞ/Y4¨Â?'†¯›ÈK?ï½ †Õ"?€¢¸•GüI?€·ÞJC;?€¢¸•GüI?ïæÍëls?L¦6Å68?i2 Y%?L¦6Å68?ïÇ#ti?{1§ÁT$?|nw1ÝÄ&?{1§ÁT$?îöF!Ȳ?«ö;rQ>'? ›ïƒtÙ?«ö;rQ>'?ïjPû4*?'ª9l5ÇÞ?'µà–Ç?'ª9l5ÇÞ?ïuRÐ1†5?|U:ësŒ?'U¥òðm?|U:ësŒAGN4FGL J2015.2-0137¿ìWQ
õÈ*À3T?Ä;-ÓÀ9+O&®ÀrÀ;¹Z%æC–@ۙC]x@™ä"rÁ?­'w-|?¹;#ÿŒ@}ÔÇm{@êñ#?ïý´'l¤¿Ù妢ì~™¿ãgwÞ]îÉ¿ä§''kþ¿ãå{ð;fÞ¿ìY!¼AGNbll3FGL J2015.2-0138PKS 2012-017?ïà+<ªç[?n|°VÖů?oÔÃe–Äê?n|°VÖů?î"šoàì?°,mZ©?­×\q9?°,mZ©?ï‡;2±A?‰o«zäð?Ž13W/½?‰o«zäð?í'ØŸ¾Ì¯?ÂÂÓu?³é;-³Š?ÂÂÓu?ï\+Sã#s?•B6ÉOE·?"z•ƒ›'¨?•B6ÉOE·?à͊ᴪ0?Ñ>N:{?Þdê<–« ?Ñ>N:{?îâ_R˜K? #ʇ±?®±ÚBÆX? #ʇ±?â9iê:­?²Rع?Úߍ,+Š¦?²RعAGN4FGL J2015.3-1432¿ëèü¦.RyÀ9›Ø8;À;`þ{›ÑÀ<º­æX@!NoæÂÂ2?ÿÌbäѦP?Ë+¿ 'Å濖HáxÞì"?ÐÀ¢\‹Ç@
°s3©OÅ¿ïà¿]x?ïúkHMw¿åL8½¶¯¿ïÿþó…õ?ïÿü¿ÙŸC¿ïÿý`éNäAGNbll3FGL J2015.3-1431NVSS J201525-143202?ïÿ™3©`ó?*ލíÕ?	³¶ÙÈì?*ލíÕ?ïé1EáûL?p/6•O÷?fιéʤI?p/6•O÷?îÄæ"Ò"? Zx.€j?£±–¶FjÌ? Zx.€j?ïÿë®Ëk4>å}ˆX¡o>äQ®(Ò>å}ˆX¡o?ïÿ<5»MÉ?ŸàUe/œ?yP|ð1Í?ŸàUe/œ?ïöƒ9Ž?"»Lâ_?‹Â_7Rd—?"»Lâ_?îïÒρn;?™¤ûƒ‹¾¤?¡ÓÅQ?™¤ûƒ‹¾¤?ïÿeF¼ä?ÑîÕ^Ó?W#~¶³?ÑîÕ^ÓAGN4FGL J2015.4+6556?áaù}Á-@0¤_¿ƒ8.À;tÿ†]À<%ü·v#s@t±ë@ËLÂPr?ßF¿¢AÞÈ?ái¥`!Rá@kÕÓ܌@ˀ"düY¿ïöµ™ª?ïd!È`¿æò
¿ ¼¹¿ê_ ®
ë¿è:´|lb¿ïþ†ܕ˜AGNfsrqS4 2015+65?ïé;o&p?tȝ'—?fĐSüׯ?tȝ'—?íDk€ñEí?»¸¾H¶¹K?µÜ£ù¿«?»¸¾H¶¹K?s:ú?•oõoþ÷Š?¤î‡—'d?•oõoþ÷Š?íãÓrÙ;?—tcÂ+ºí?°ç¡fŽ÷¢?—tcÂ+ºí?ˆ',µ?™6K%EÜ?]ͶbÅ?™6K%EÜ?âMŸ'£,?ÓDŽåh¶3?ÛdÁ°¹ñ©?ÓDŽåh¶3?í™ÿ^ß"?¥'Î
'\?·Û0Rál?¥'Î
'\?×æA1<|Í?ÁØåó?äßgaÁš?ÁØåóMIXED4FGL J2015.5+3710?륛N¿D"?óFç_ö	ÝÀ7OE0‹¹À9¼°´hQù@ 5ä¾[@¤H)í?¦~qcß<U?ÆÀtå/D;@"vtÑc5@TÊH8(¿Ü	"(™&¿Þß9K{(•¿áˆ\ZséÝ¿æj>B(¿ë'"ÂÀ'¿ížè]RlAGNFSRQ3FGL J2015.6+3709MG2 J201534+3710?áYµ
(n?Ô`÷s‹à@?ÝL•Íå¯$?Ô`÷s‹à@?Ê¡zŸ¿‰©?ÏÆx]<y·?éW¡X–?ÏÆx]<y·?Ý\ÊUú˜?µBl@ðàþ?áQšÕü4?µBl@ðàþ?ྤH§Â?Ãúz,õ_?ß؂·n°|?Ãúz,õ_?Ï<˜â¾?ÌÉYHW?è0ÙÇ\'?ÌÉYHW?žLŒ‡Æ?³ON¯>D?ï
Ÿ;€Dð?³ON¯>D?ݜ¾"ec?¾†?y‹°?á1 ønÍN?¾†?y‹°?"C½Ÿ&Y-?"³f~¢?ï]â0†?"³f~¢MIXED4FGL J2016.3-2331?éIˆ½±ÚaÀ<†·þ®ûÀ:Ò<!~|À<°¹ßŠ>³@˜¥àyÒÕ?ÿï¤h)µ?ÉÎu™_7?àc·_}>@N1ÿVŒÕ?û[(g¨/ß¿éò^VÍl/¿Ëº!úP¾‰¿Ð2!zÎþ*¿àY	†'¿îZµUů¿âþ@Bæ/AGNbcu1RXS J201604.8-233049?àë#g8Hq?ÉعVÅ«é?Þ)¹1o?ÉعVÅ«é?åj¡†Fx?Êÿí«¿‹ò?Õ*½Ôós?Êÿí«¿‹ò?ålöÞæ?µS—z9@?ÕÍ'ÒB3?µS—z9@?çï
¡³Ö?ª¬#àµ
?Ð!åÖ¼˜U?ª¬#àµ
?Îhw~¢Ùp?ÃÉ	`Z?èeâ WI¤?ÃÉ	`Z?Ã
Õö¶?Æ\C¢ÂT?ë<Š'O{?Æ\C¢ÂT?Æ/9µJ?µ<<ê֝è?êt8q¿®?µ<<ê֝è?Îø`4¯E?´¢"êSÿ?èzçòÔ/?´¢"êSÿMIXED4FGL J2016.3-0903¿ï`2j`qÀ6÷ƒ8.D·À96œò®3À;ÃÖPM'@²ÐG«<?ý¸¸É	É­?®ØŸ¾Ì®ð?µ«½ž¹þ@ŸIc÷ ]@+3¥Cò?ïó?Ýæzž¿ÚS°àˆ¿ÚsŸŸB%¿àáö?6÷Ž¿ÝåÌ¿çÀÞLQkAGNbll3FGL J2016.4-0905PMN J2016-0903?ïümݺA?ZßÑAg²£?<'ä«Ú‹?ZßÑAg²£?ïØÞÁ
X?v´P‡]?sŸ'	W´?v´P‡]?ïÜ\mêË?tzR42ë?qÑÉb<fµ?tzR42ë?ïäsö®î?O±þ¦ÌÑ?kŒ	y؉q?O±þ¦ÌÑ?ïøt¾Ìa¡?G›^ãYø?N-Ys?G›^ãYø?ïC*¸û?§QF®5?žwš³x|Ž?§QF®5?ïÂcÚÅÞÇ?€¨@Ylü?~Ξptƒ?€¨@Ylü?ï¯Ó±‡:á?mº5ã•%?"­O¥?mº5ã•%AGN4FGL J2017.5-4113?Ã4֎'À@µA•Ì…À:'~Ù#óÀ<yÌí€@ Á-Ý2ö?þ¡™'ƒÒˆ?Á†~Ëb?¶æMý8ûI?ö¹Ö ‹%c@•èO	R?ïŒo_3l>?²Xúm¿Ú|²ÙÀ3¿àÎ1†ŠÉ¿ßÂLì¿äڅ‡"ݘAGNbcu3FGL J2017.6-4110SUMSS J201729-411516?ïÿ{ÆÓl,?ÿ!΂L?‡g"t<?ÿ!΂L?ïñÑyB?h°tˆ…Mœ?\]Ñ&®¬…?h°tˆ…Mœ?ïïf«8[?q~¨¹?`™Tÿþ~Ô?q~¨¹?ïø1T‹Èv?2ËÆ%óÿ?O:­gÝM0?2ËÆ%óÿ?ïÿ^3Uܚ?/-S´o9?9"6ÓÎ?/-S´o9?ïØ×ðÊán?v!ƒ~î?s"ºÛœí?v!ƒ~î?ïï`ñp?q6(e	Ô?`Ÿá
Ià6?q6(e	Ô?ïèš×˜hþ?TyB£ÄÒ?ge(]øá?TyB£ÄÒAGN4FGL J2017.5-3753¿î?ï,¯F»À@E*"8…À;ñ¤óiðÀ<Ö)làÔ@VæÌzm?ý
v
HX?Ôá5"Ç$—?ыt¨H‰?ûLv›gÏó@E¼uÎ.¿Ú?%ðz|?ïïUÑ{¿ÖÝ~`X/l¿áвÀ12þ¿ßݜÞr'˜¿ïÿý¡UûŠAGNbllPKS 2014-380?ïùb}´ÇÚ?RÄu"Ýt?JvÞC#ö?RÄu"Ýt?ïÙoüxr>?}E"dðAá?sHÕ¤Ù?}E"dðAá?ï_&³Ò?†—ìí¿ç?"_yq·Ò?†—ìí¿ç?ïñõ® ð?D[Z¦ìԌ?]Ú"ÿ¯b?D[Z¦ìԌ?ïûU‹D8¶?H(±Xm?B©Òðð?H(±Xm?îߧ4âµÂ?°*-Í€?¢Œ®eá?°*-Í€?ï^ÊÄÅþc?'Œü—«ö?"&§j¯Ï¦?'Œü—«ö?ïҊðùÅ?lE2›Ôùi?vº‡w…¨?lE2›ÔùiAGN4FGL J2018.5+3852?ÖÎNãÏ?ú¬løQÀ9zeEÔöÀ;Œ 4Rî@ ²þ¤‹:0?ý5¤ãc?À"úˆÇº>?Ò2¿-{@
}ܤ±$Ñ@󟳏%¿è.Ê榓¿éàz~¡Eµ¿½yG'R¿Îk~¾¡æÅ¿ãÊ^'Ӄ ¿ë–BAn	sAGNbcu3FGL J2018.5+3851TXS 2016+386?ï(¨-Ž·?î1¼ß›'?šêúQ˜¸™?î1¼ß›'?î˜C^,8Ì?¬{ÔçÂT?¦{ÊZD?¬{ÔçÂT?ìèg"ÆK?¥OdÞÃ$?¸¿|ÇÅ´§?¥OdÞÃ$?î§õP_Ð?…¿ y¸¡É?¥€ªö"c­?…¿ y¸¡É?ìQ/×wåY?µOÔ€W(?½vD@Õ;?µOÔ€W(?è*zó'2?ËëŸuѓ?ÏWâ1»9?ËëŸuѓ?êûöÜsfˆ?¬9ƒs+_™?Ä$Ž2eá?¬9ƒs+_™?èl.ÙK$/?²UŒ»šn?ÎODšÓoB?²UŒ»šnAGN4FGL J2021.9+0629?é¥ÃOÝÌÀ0Çñ"<:CÀ9Ô¦ló"À<›ûs©E@hþŸ'¼³?ÿ8B·4µ?ÁzØù«Ó?ÃW"üÑÍ=@uîþOý@s''dç?ïùd:<;ð¿ÜÔ¬ÀþZ¿Ú­.â@§e¿Ý•+uϐ¿ç6‡æ鮅¿æ䡟øXlAGNbll3FGL J2021.9+0630PMN J2021+0628?ïè΃X"?¢æèS9Y?g1}<Ÿû)?¢æèS9Y?ﲬ[y^¢?h!ÿ
¤Ÿ?ƒTéñɚ?h!ÿ
¤Ÿ?ïÕ|±lÒ?u¡>a	9K?uA§U÷Ø?u¡>a	9K?ï]Ôá2#X?rÓþ¤ö?"EcÒÜ]?rÓþ¤ö?ïÂL2U	>?~''iLƒ?~ÙæõÇ´¶?~''iLƒ?íí@Š‰±?¹|¼ù?°—ùóäx?¹|¼ù?î°U
ߢÏ?Á5Ý
]?¤ú¯–7?Á5Ý
]?í–ésvš;?–ý_ëÌô?³H´e'%?–ý_ëÌôAGN4FGL J2022.0-7224¿ÎëÀ|v7À@H6âëÀ;_~À<½~«Ê@!"˜`©G?ù§»/ìVÖ?Íҟ_+^©?ÊâÙih7?þǧÓï?ûðSå…U¿è"'|É?ïèw'î\j¿â
Lõ|¿Ä›Ï¿Ez³¿åY"‰ê¿ÄãA-qÓAGNbcu3FGL J2022.2-72201RXS J202204.8-722538?ïüÆî+S?,ٔ¦vâ,?9ȍ²"¿?,ٔ¦vâ,?ïÜýF'5¢?yh=¬4?q\©Ö«?yh=¬4?ïÓÛnr›Ë?n½+Ó!?vHÞ¿^<?n½+Ó!?ïÃ.áÈe?bþ"ýÕ\)?~h-O&?bþ"ýÕ\)?ïú'ÚĘ\?@ý9ÿª?E¸•D{¢?@ý9ÿª?ïx}[˜?™E÷jŒ6?ì\iuU?™E÷jŒ6?ïÈoâTã ?~Ƌ¨´Ñ?{ÈãLßå?~Ƌ¨´Ñ?î¾
bë˜Ñ?'êiªcwf?¤Yβ½ó?'êiªcwfAGN4FGL J2022.3-4513¿ïéñJÛpÀA;—ædNÀ9•s³VBÀ<þ+êi–@±ß*óH·@+sKQ7*?°šï¯û°»?¹ü¨ ‰Ò@	1eәo¨@§@,ÀÓ?ïö+ÖGŸÒ¿ÔçÃK•U¿áÃ1­÷õp¿ãmOŽ³ŒŠ¿çätôž¢î¿×|0}d/AGNbll3FGL J2022.2-4515PMN J2022-4513?ïþ=}dá?-¿uBĘ?,(,à3¿Ñ?-¿uBĘ?ïñÑ«½•?kÜ'™.2@?\\©×öt?kÜ'™.2@?ïÝúÀŒ2å?rì³ÍÅkÀ?qŸ«x1Ÿ?rì³ÍÅkÀ?ïú×muàh?-)t7iÒ?D¢Iêê?-)t7iÒ?ïþfÜ)À?(`«Î>?)—!!·zÃ?(`«Î>?ïÓh"Ó?…¨…F…³?vqKªÌêx?…¨…F…³?﮲¤Ձ?ƒ™B+R¤ø?"SW™s¹?ƒ™B+R¤ø?ïð1Ð?LUó#ë?_ÑÏÖnË?LUó#ëAGN4FGL J2022.5+7612¿éC¡Êˆ@5#1;â.^À8éÃ5tVÀ<²<'Î@ÇäX¯™‹@íòœj.r?¤Ò' ½ÿn?¡ñrsï¢?ùÿ¢È"§@oÃgp~?ïÏ"‡"‰¿àâ¢Â7G•¿ä»dàTi¿âA3¦ö¿åÍ·þßn¿åòGAGNbll3FGL J2022.5+7612S5 2023+760?ïþ—(aYH?Á†J)?&yü!~?Á†J)?ïój=`ˆ¬?^>uÂÅ?Y+…x¨ï?^>uÂÅ?ïïƒî?q®æ3XxŽ?`óú§"9Ô?q®æ3XxŽ?ïõ´ä	¯?F¯ÔûsP±?T–880â?F¯ÔûsP±?ïþ"Ìî?#¼qÆ·ˆ¡?-ÓB'|
Q?#¼qÆ·ˆ¡?ïÆ|'¡IU?…iÈôå•}?|Á¾¨|x?…iÈôå•}?ïé¹½¯<?tÒ¸}<Ë?fFBh]?tÒ¸}<Ë?ïí=c@tÃ?Up›'zèë?bœ±ÌÍ@?Up›'zèëAGN4FGL J2023.2+3153¿äþŸvcšÀÀ½gý?[`À9¡ §?tŠÀ;oÆÐ3‰š@!]´8×7	@qú[{PÙ?¾lðï÷ä?¤R×¾Bph?ênwÂYV^@lF__áè?Ö£e_Ö)m?ï±ß`£-í¿Ù¢'ÌM¡¿âç!A™'"¿Û؜cÎ[˜¿á‹ºžLèAGNbcu3FGL J2023.2+31544C +31.56?ïøéëö;?A±µKGe‹?L[õÐA[?A±µKGe‹?ïÊË´ãÍ?"îsËÊ?zš%›F@?"îsËÊ?ïÎb…þ~˜?{ٖaéB'?xμåCÔ%?{ٖaéB'?ï˜ø[=¥?s¾uÜO?‰ÁÛÞáÂë?s¾uÜO?ïØ,ðVN?rƒ¾Š¢g?sé‡Ôlå?rƒ¾Š¢g?ï'çÔÚ?§ka™jM:?›Ã¯¾È?§ka™jM:?ïPôöG֕?"‰Ò"‹
?•áa:tÉj?"‰Ò"‹
?îN¯[çv?›N"-a«?«åö£?›N"-a«AGN4FGL J2023.4+4127¿çò}ú	y"@Õü¦¯+ÒÀ8ÿÊñ*z'À:ÕKoj'@ wýFKê@Œ~»ÇÁË?Áõ…Rº·÷?Ä·Xtû@B"~ea@wóòUk¿ïÿôa¼2¡?ïÿ
ÂPÇï¿×£aÔÜ;¿â(orŒ¿èќªÆÈ¿Ý#®ÆQˆ‰AGNbcu3FGL J2023.5+4126SSTSL2 J202336.19+412527.0?í ¡ê1GÝ?Æ~Òðõ˜j?¶úð­+æ›?Æ~Òðõ˜j?K´?«¥ÍY"[?¥ÞFùŒéö?«¥ÍY"[?ìYã1y[?©£ëq£Í?»õ0æt5(?©£ëq£Í?íű‹¹î4?˜}k‰†"?±Òs£u^?˜}k‰†"?ݱ¿‡É?Íoq1Ævœ?áv' w¼?Íoq1Ævœ?è¥ñ½á¼7?͖ÕöRhi?Íh9y$?͖ÕöRhi?å5÷ç?¹–…Úæ1?ՔÒ1Ýë?¹–…Úæ1?ãó͒Î?¿n\ibT?ØdÚcýð?¿n\ibTMIXED4FGL J2023.6-1139?×vSʾÛÀ9­Ð¦v ïÀ9Y´Ñ-"žÀ;õSì^ó@w#Ñ@yî?ÿc<Ù¥"?¯·Úø3­×?À­aw"6-@ã9:´0õ@
w헝•þ?ïÿ¦n£¿½eøØCx{¿â<XuâÛ¿à¹_²˜¿åë'H'@	¿í'¦ïnAGNfsrq3FGL J2023.6-1139PMN J2023-1140?ï÷—á*Y?QAuä†C{?PÐ>6-d?QAuä†C{?ïq‰(Ììœ?˜óbgó,?'ÎÚ䪞?˜óbgó,?ï›räÆ`?†ƒ¹¯âÒ?‰#FÀ©‰ï?†ƒ¹¯âÒ?ï;fâ}%?ztÁ ÝÍQ?˜"#¾)h?ztÁ ÝÍQ?ï˞èŸ!?}2K÷Ž80?z0‹ÍûäN?}2K÷Ž80?ëÔ°Èyá?Ħ𼍇?À­<Þ˜|?Ħ𼍇?ï$¥²?–jgó\?›|+AÆm?–jgó\?ìWOŽ¢^~?¤™¬FÁò?½EƒŠí?¤™¬FÁòAGN4FGL J2023.6-0123?É]ȒÖ[íÀ5þ÷ÂDÀ:[§ŠóäÀ<U›ÍP€K@ÁË[ˆ'ß@Íp`»?ÂeãØ×ó?ם 6×,¢@ÏÄ~I±û@ù(uj?ïöŸ>I;Þ¿ÓG>'òŽ¿Þh3Æ)ñ¿â¡ÎAÒ¿î@;#Â|è¿ÕS"g*±"AGNbcuPMN J2023-0123?ÕÙn~ÁY°?ÇÎk­?åHÀŸS(?ÇÎk­?ê0eA¼ý'?Ä»ƒE¼š?Ç>jù	½?Ä»ƒE¼š?â€];"?¶ÞèšÕü?ÛÐÿE‰»Å?¶ÞèšÕü?ì<Ñ'á'?—ÏP¦.Õ
?¿FvÀóó?—ÏP¦.Õ
?·›è¥Ü£#?µ)@Äò
?í'ë_è|?µ)@Äò
?Ë¡¢ØîªS?ÉÕ4*æß?é—IÄUk?ÉÕ4*æß?¹%˜¶×í?¨Ïâ¨l [?ìÛLèøÓ?¨Ïâ¨l [?܈8ß«²Ý?·BkY@@?á»ã*&'?·BkY@@MIXED4FGL J2023.8-4828?åã?!uhÀAz»˜Çâ'À;L-ê
ËÀ<°ìˆ3@@CÁNêHß?ÿû©Y*=Á?ÑØ
¢gÉ?±ÉòQì†Ñ?Úµò€:¢é?ÿ·	Øi
?ê0‰jwm¿ï5§¡ïÿW?ÝÊ3)ø÷οÜĄ¿Aô¿ïþÍ?äF'?ïõ@‰]tAGNbllPMN J2023-4826?ïön¤M|¶?^UzòkÃ?S"·à¸"D?^UzòkÃ?ïô2îـÔ?X‡L"`?Wš"9À‡ñ?X‡L"`?ï†iÖ0?…#7k?Že»ã—?…#7k?ïó&v>ÿ"?Lºh;Úi?Y³¢ýü?Lºh;Úi?ïü¾7fQK?C÷"yps0?:Fí·Âf?C÷"yps0?ïÈ,{Ö\?†ª'÷TXô?{éÂ.î¿ä?†ª'÷TXô?ï¦XÔØ^ü?ˆŸbH"?†iÊÔ7ã?ˆŸbH"?ïՈ>
½ê?pžSH¬?u;á`þ?pžSH¬AGN4FGL J2024.4-0847¿áŽUÌBíÀ8¥"¦óõ0À9Ë,´"ðãÀ<#:Š?‰ƒ@ £Y5ü?ÿ!{zÊ¡y?¹×Ó2Ó?ªñÆ+rõk?ñˆڀ·@ùyŠ˜?íbfâ(r¿Ùuã'¥¿âg…_ÐË	¿Ü%l 9±R¿Ü
EbàŸè¿è©rÀü¨AGNbll3FGL J2024.4-08481RXS J202428.9-084810?ïú¥Óí0"?:EMx©?Eh°®â?:EMx©?ïãBYŽ3+?oÉꞴ«'?l½¦~+l|?oÉꞴ«'?ïìW…å?e3,È?cî¨g±JÖ?e3,È?ïÓyʋ?\·á¼ö¦r?vzC'È÷û?\·á¼ö¦r?ï룬[Ø?]WÌ×ø´?d÷\€~?]WÌ×ø´?ïXp'Q²?Ÿ‰tÞNTw?"ñï­2¹Í?Ÿ‰tÞNTw?ïƬKÅGÀ?"DnŸ©?|©Ú2©´?"DnŸ©?ïu\ƒ8¯?yøj,í?'To'
äH?yøj,íAGN4FGL J2024.6-3252¿ï™=´À@rö@c^À9[ù‹q¸ªÀ<YhQ"2@'ÝžVAÖ@хÞz?²#Š•š±?Ã}ƒa@êÿÓ>×@¸	™¿Ø¢PA¶Ù›¿ß	Û !³"¿çqž]£Ÿ,¿æªõwÖ¿é¼]°	s¿ïÿ³©æ÷AGNfsrq3FGL J2024.4-3254PKS 2021-330?ïø"ŐÝ!?Jjð" 1?Mìꥤ,Ñ?Jjð" 1?ïÜßG+kF?'ÔIùU?q\Iþ	?'ÔIùU?ï«{.œ\?~ žYœp?…!:ôXé?~ žYœp?ïô›{y¦"??ÍO†mã¼?VÉ	>-:]??ÍO†mã¼?ïêí("Oþ?`Å® ?e׶ÉIò?`Å® ?ï1`vÒ:?£ÏÜ­hÏ?™Óñ%¾øÆ?£ÏÜ­hÏ?îç˜-fs/?˜%5™"ç?¡†}'?˜%5™"ç?ï̪°_?h^
Ï <z?yÀ*²ó:?h^
Ï <zAGN4FGL J2024.7-2328?Á'¨MðŒÀ>Rk?éúÛÀ:¿ìMøÀ<€¾‰¬½@o¯YIre?ÿ3-Ú-Þ`?ÉõDæf?ʬ¬è*÷@&ûëýê@ÓÊJ¼?ëM¾,0
?ï]ËB83¿â›6A°y…¿ÜÊ®DK‰k¿å5¯¿ ¿S¿ïÿý¡UûŠAGNbcu3FGL J2024.8-2331NVSS J202442-232826?ïò8ÌF·l?]›b]¡~?[Žg3XXš?]›b]¡~?ïÆM|_¡ü?†+ª÷¼™â?|ÙA¯2Â$?†+ª÷¼™â?ïžçoÌ|×?ˆ18½!8?ˆF$'öO?ˆ18½!8?ï~©`-‰?u!õ{s:?*Óöß0W?u!õ{s:?ïÕëŸJÞv?tÌεe>'?u
0e…%?tÌεe>'?îg"s—§?±Öã82?§)‡»Z:‡?±Öã82?ïPW8ÿƒŒ?''lÉ?•õÚè$‰?''lÉ?î
íÇvÕ?Ÿ² Ø?¯'!&Gª?Ÿ² ØAGN4FGL J2024.8-6459¿ßLòšo`ÀA'žÓ•>À:ˆ¨½ùË3À<†\S½í6@%ÄRTá"@(\ÅÓ´?¼øӐá9@?£cV9?äÄ°¾Ï3/@ÅÛAÖ?ïý@h¿Ûšðü××m¿é6ù5¿ã‡!A™'"¿ãmÝô<}_¿éMOõ^fAGNbcuPMN J2024-6458?ïýâȦfJ?A‡T‹gÅ?0é¸Üìu:?A‡T‹gÅ?ïöÙ=üî[?X×ö¤÷­?RM"fXXï?X×ö¤÷­?ïÙø|²·?|°¸àz_?s÷PÄì–?|°¸àz_?ïÿx£ª¿‡>ûhhg5À|?ë"\œ>ûhhg5À|?ïýÁÁxRD?4]&Æ'Ò¡?1ñõ8.è?4]&Æ'Ò¡?ïÛ5Þçµ?'­4>ªõ?reŠÅ ó?'­4>ªõ?ïÐ5sÄÍ?€°\»Ú¥?wåFYñ"?€°\»Ú¥?ïþ¡®fl?ú,¢®m]?%嘕òk?ú,¢®m]AGN4FGL J2025.2+0317¿ïúýÏÏ
ÀÀ3`4óþÀ9:yÂc½?À<®Bž
B@gÑØÐ;A@†ÛPô?®h¼ày/Ÿ?³‹ÉLd²‡@çÖs>»ý@«é¯¼'¿ÜFï}¦ÉÙ¿ßða<æ¿ã«DAM}6¿ß¥Iû÷‡¶¿çnÅ°xÙ¿èç(bõ˜žAGNfsrqPKS 2022+031?ïþƒa°{?4ÓGø0j?'Éåè¾a?4ÓGø0j?ïÛ«ÜV"?€¦wúÀ¬?r*ÍcÞ?€¦wúÀ¬?ïðLÅÅ5n?^ì™ý\Ú?_ftëÇ´>?^ì™ý\Ú?ïü´Ý?+e£X@Ë??§ëÓNê¸?+e£X@Ë?ïýy&vP-?04êÕj—¹?46ÍPú®Ã?04êÕj—¹?ï–«¨×?©2f ò-?œ
*Ž]¡'?©2f ò-?ïÉZ'`®?€z+áÎpJ?{R¾Ïð)?€z+áÎpJ?ï÷2ôw?B"Ô­+We?Q›ò-Gé?B"Ô­+WeAGN4FGL J2025.3-2231¿êBŒÜ5º;À>"ÓÍ$áÀ:‹Ú¨W¢À<nU•]ʶ@ '6Ö*ïm?ýégØVmË?À¦´_B°ª?±Ìö%‹«?óá3ÁÎl	?ù»fØ&G?ï÷ڂû¿ÜªWA…[t¿Ý¯ïüý—¿ÑÙ÷¢äF¿èíòKâV¢¿|>ûq-AGNbcuNVSS J202515-223016?ïæk˜:°?mH'P‡$u?i"güI¯O?mH'P‡$u?﵉©X÷?ˆÈ—©—x?'¾]'Š:Y?ˆÈ—©—x?ï{»µD½?‰íô® äR?œÈ‹6V?‰íô® äR?ïïÃFç?ÝÁñ5d¡?—#»?ÝÁñ5d¡?ïb?ý4ãP?e
{¿3?"¸aú›è?e
{¿3?
fƒ?¶Æ÷C'†?¯´UíLÑ?¶Æ÷C'†?ï%m®•ei?"oAæ±"Ã?›RJ(+èó?"oAæ±"Ã?ì'
l&?¦ßx"¢ÆÒ?¿fǬžÑ?¦ßx"¢ÆÒAGN4FGL J2025.3+3341¿ä•ÔZµ®"ÀR

ù¾À8A=e¼{À:™-BŠ¿@‡/›#1ˆ@Ò±-4±?²jî «†?ÆÖhA‡ß³@s ÔƖ@ÉÃØÝQ?ïÎxžwNì¿å«ã‰o€¿çý"såªê¿ç8?!(οï-ád´`¿Æƒ~_pAGNbll3FGL J2025.2+3340B2 2023+33?ì+ÙUNð?Ð×kn!?¿F¡5Uˆ"?Ð×kn!?ïµM:'?¤H'eÔ¸W?¿©[€Æ?¤H'eÔ¸W?édF½úÖ?°×ð2Ö·Ÿ?ÊnåÄ©?°×ð2Ö·Ÿ?ï0%ÿeá?ƒ	2¢¢Sh?™û@
ƒ§ð?ƒ	2¢¢Sh?ï/Gµeó?N½¼ßOù?š	Q¥sž?N½¼ßOù?êUõCI¼ô?ÊCÒ,æœ?ƨ*òÙ1?ÊCÒ,æœ?çéÌÿ‰?²»–R>«?ÑÞ-öfî?²»–R>«?æ·E·¢Ì§?¶¼ì´7™c?ґtºf³?¶¼ì´7™cAGN4FGL J2025.6-0735?æ\©»ÈÀ8cY§TmÀ7"§&J¥À;;A¼bò>@t‹gÒ¢$@ƒÅ_AË?Žµë`ðR?¸ÝÊ @&sü"$íö@ Bî «†¿Ð7X[á¨&¿à9RÂÀp¿ä¸;æ`Ê¿åýÉÄڐ¿è½jęød¿ëS/uKAGNfsrq3FGL J2025.6-0736PKS 2023-07?ïêõC?k%.O)!!?er
ʹk)?k%.O)!!?ï†A<'´?¦?gá«?Žo°ßRØ·?¦?gá«?ïÏg·dÅ?}fñ%ǏÌ?xL$y¼™v?}fñ%ǏÌ?ïóí](i?X",Àý߈?X%Ó$²îQ?X",Àý߈?ïßÿÏ?kF™"û¥?psv—#"'?kF™"û¥?í@ù!"zK?đK;V‡?µø6ô¦'?đK;V‡?ï³ê
'ýÿ?‡Yc³(—ì?ƒ|›Ðä0?‡Yc³(—ì?ïŸJe©Òø?ê0ÕÉÂJ?ˆ-f˜úÞ?ê0ÕÉÂJAGN4FGL J2026.0-2845¿Ö7ùÁw"À@"ƒ‡ß]À:˜i6$;À<Míض@HLó"Ìß@dqcðja?͘+ˆy?ŜÆʪ2Ä?ö–•ˆ'á@	Þ'h#ֿ湓¿ºëy¿âÇ`Ƥj¿èýب£!Ù¿è"u'À²¿è¼ÕÞÄF¿ïÿ½ÅGóAGNfsrq1FGL J2025.9-2852PMN J2025-2845?ïøHþ˜ï?V%žˆ^cY?NÜÑô*!?V%žˆ^cY?ïç"4/?p¦6'?hçkoËÑ?p¦6'?ï³Y²Š¢?F'EQ‹?ƒ)"S"¹o?F'EQ‹?ïö‰ÿÈ¢œ?;!j,³œ?Rì@ÿ?;!j,³œ?ïøío¸'W?Mf3{5gâ?LJAæòY¿?Mf3{5gâ?ïx7¦#Y?˜½@ýFc?ù8%1ÿ?˜½@ýFc?ï=aVJÿ?'6äΊ?˜SÕ.	™?'6äΊ?ïÆ,â·Ý?n}µ,.›?|鎨'™j?n}µ,.›AGN4FGL J2026.1+7645¿ïü¸Tg,×@59>ê ›À;
æ_E	õÀ<«­	¸æf@"Š[Ö?'<?ø›%:L,(?ǝ¤ÖŽ—ˆ?ÆWe—‰t@‡ÿÞr¿@T=ïϱ¿ïëUN.K¿ï×ßàzԈ?ïå³vQì?Âv'^¿à´€€G¿¾³ÌÓ¯ëAGNbcu3FGL J2026.3+76442MASS J20263126+7644487?ïý(JÞë?+>ԂZ?6½§p3_?+>ԂZ?ïîI}ç%W?b²Kǟ«r?a¶'Q4@F?b²Kǟ«r?ïíýÎÄÁ?O³ûD¶?b0ýfC?O³ûD¶?ïÐ !f4Æ?dáD­ë
?wïïZ¤û?dáD­ë
?ïû/Æ8«e?9Oz²'Ö?C@çò 'ì?9Oz²'Ö?ï².ë>â?ŠøGh¹Ð?ƒtE2'"?ŠøGh¹Ð?ïär=è¡r?s¤iÎE2è?kÁëcŽ	?s¤iÎE2è?ïs'Y'õ>?†¤]LIJE?'´Ô 5?†¤]LIJEAGN4FGL J2026.6+3449?×͍™ÂE¿ÿu
xŽ‡À9¢ZÐ0.œÀ;?Ö§A"	@ s¹£¥60@CÂÍoŠ?Â8Éu)wÉ?£ùÉÁ:ف?âUKÚt?ý3ßJӸϿîÓAáKßÒ?îj»_¼þù¿è`¼mÙø.¿Þû]Ay¿ã–,A§j=¿ç¡®pÁ3<AGNbcuNVSS J202638+345022?ï÷b.•·?EìJìtð?Q;£L©
?EìJìtð?ï~+"py?›½[>5?:‹˜8?›½[>5?ïžÿoÈv?†ƒÂËIÈ?ˆ€.\¶o?†ƒÂËIÈ?ïCK,µPë?úHý;&â?—–šbvª?úHý;&â?ï¸L÷nOÙ?€ÖpÂdY?ìÂ32[Ä?€ÖpÂdY?퉡Rã?¿Ê¥HWd?³²÷¡}6ä?¿Ê¥HWd?î—U$Au?Ÿ•$ľ2?¦Š®Í»è­?Ÿ•$ľ2?êëÔù°ÊR?²¢ðÙ$&®?ÄP¬<Öº?²¢ðÙ$&®AGN4FGL J2029.1-1839?æ®Od¨\fÀ=£·•-#OÀ:°dPâp£À<kَ|/&@ˆ>	P
Ú@ÙaÃiv¼?Íe˜¶×í?Ó@ª; g@EQÄ?ÿc‡ÁÕÍÒ?ïßÓ™hF¿Õú,@ûÆ¿äTž›·¿åÿ`h¤
¿åU'ÿùJ¿ïÿqšw+AGNbcu1FGL J2029.0-1840NVSS J202900-183709?ï¹CTW^û?G7fê?¯*í—Ý'?G7fê?îù'½µÕ?¤ °²a|ø? gÔ%‹É°?¤ °²a|ø?ï
AºŠö?'"–V`bU?ž·È·G.?'"–V`bU?î`źVJ?ˆŒµÒ× 2?©ó¤Z›_ ?ˆŒµÒ× 2?ïZÂE¶Æ?'n_ÌFÔ¡?"§·G2!C?'n_ÌFÔ¡?æžÈ¬ùë
?ÐX|Óvp?ÒÂn¦)ë?ÐX|Óvp?ìÙM\1â¯?©6ú†ýg?¹5•'?©6ú†ýg?ç–û¦÷H?²%¦YèËþ?ÑàÒ²q?²%¦YèËþAGN4FGL J2029.5+4925?†øMÿÉ@ª@]wúã`À9õ6À;jÍë°½£@´Øö¦ºê@×R9ˆ·Ê?¶ÌMöØäÞ?ÓA­§m˜@ÙgÊêt~@ó,ª-®?è$ÁUuR¿É/¥ßøù|¿áÓ+UïÞ¿èì›Sþ¿ëF–½FG¿ïø3þ_AAGNbll3FGL J2029.4+4923MG4 J202932+4925?ìbSPxØ?µC_‰Õ
Ç?¼íe|9??µC_‰Õ
Ç?ËÓ'°?œº?2n1ú?ŒØÌýw¤!?œº?2n1ú?äï¥G€P?³X‰'$*8?ÖÄ µpÿ`?³X‰'$*8?ï©Æ°Sƒ?pvõç?…ŽSÝ{/q?pvõç?æàd¦•"?ÆX%25ÿŽ?ÒÞ?6²Õ¼?ÆX%25ÿŽ?íFïÉã¯?Á^§âÿáo?µÈ°#‰?Á^§âÿáo?á¬ÏjG,Ë?º¯3¬!?ܦa+q¦i?º¯3¬!?íï~´Õ£û?˜þKª5c³?°"
Zœº©?˜þKª5c³AGN4FGL J2030.2-0620?á{sâ-¹À8Ö®::ŽqÀ:GÖ(ôìÀ<%o•º@ǯïœZ"@qƜ1#Ž?º…࿝å.¿¨>,œ§QN?êG±ÚØÿ
@C×n;qñ?æ*K-$ü9¿à
è`ܺ¿é·<­/x"¿ÜÞ>ÄáÆÚ¿êˆe>É…¿Ä5»"ÖCÄAGNfsrq3FGL J2030.2-0622TXS 2027-065?î·Q]¿?Æ("ÁÎʆ?¤ŠîœZˆ?Æ("ÁÎʆ?ïæ¿ÝP'¶?sš¿´Ë£?i@"³÷ÒT?sš¿´Ë£?ï°gí,Ç<?ˆV¬ìû?ƒæ´v;?ˆV¬ìû?ïÿȕIm?	6ŽK€cr?æðöÏMt?	6ŽK€cr?ïóÀÇ?Y,Ø9ã1°?X¹;¶?Y,Ø9ã1°?ït"
·µ?œ)lk×ø?'mŸ¡¸¥b?œ)lk×ø?ï±sI…õ?†éùX¾U?ƒ£8c§¤ß?†éùX¾U?ïüûw ?,P›+ãù ?8'[HOA*?,P›+ãù AGN4FGL J2030.4-0502¿åù*g¡iÀ8Lma,jÂÀ;,,"ÜÁ7À<ƒØÐç
Á@ ZÑÜV,²?ÿ•;fœ?Ñw'w?«)ˆ9ŸÞØ?áj‡þf¢Ì@'šËrړ¿Çӈé:x¿ìxþžÖð<¿áÿ®ÁžñG¿à
ïAkÛ¿Öµ»€Ê¿á·1$e:AGNfsrqTXS 2027-052?ïþæÝÅ¢?æàׁ?!' ¨w'¨?æàׁ?ïèMÉXñU?n2†¼¹ž?g²6¶,ò±?n2†¼¹ž?ïô¼»€Ž?V:á3~`?V‡þ&
$¢?V:á3~`?ïý]…U? ˏ³"æ•?7]©f\? ˏ³"æ•?ïÿô÷õV?"™a¹^?!f–²Ày?"™a¹^?ã[Ò?'[A?'?—ÿwß{?'[A?'?ïô0›u´/?c€´Žô[?WžÉ	˜âê?c€´Žô[?ïñÀ¾ ˜?PmÐ÷TŽæ?\Ì\C0¯?PmÐ÷TŽæAGN4FGL J2030.5-1439?Ün(ýzÀ<o"}cÀ:¶Fà‡•À<yŒ†‹ŸÜ@ çþ¥aùÅ?ý©•?ÇR¡ãj?žŸyzÀ;?Øß#¦@@víb£æ?å•6Þcx¿è»îQ"ñ¿àÍ,¾¤ëݿׄH"S6^¿ÏU-Ä^iB¿ÕC¿ÝÑAGNfsrq3FGL J2030.5-1439NVSS J203028-143918?ïüUØh{-?3CVùȲ?=Q<·À®'?3CVùȲ?ï鿦¿{?o•X.®?f@ñz<ÅK?o•X.®?ïïOÈâ~Ý?]¶Í¯?`°6çç;(?]¶Í¯?ïùoýâ?0ïµëçè?J@åè?0ïµëçè?ïù0@ö¦v?A‰Ü¶]è¶?K>û"¶¸?A‰Ü¶]è¶?i>'?"ç1ø¬–Ð?^¥Ÿ-ϓ?"ç1ø¬–Ð?ïðºÀä>â?d³sdò?^Š~E@¬?d³sdò?ïë
ºîþÑ?T´a$iã?dõDæfe?T´a$iãAGN4FGL J2030.8-6959¿ÑË2Id‰(À@ç]þ¸Ø#À;¨mqóbÀ<²˜§+R"@WR
é͏@ځNš?̧ jْ®?²ú2¡ì?äyºHeÊ@ßËZ'œ?íqD îÍ~¿ìKIt¾þ¿ÅCŽõü›ò¿ç.ðäJ7¿ÜEva†,Õ¿âg¡yâÅAGNbcuPKS 2024-701?ïþYâŸqö?"z/3ÝÇ®?*aÕÚ²±R?"z/3ÝÇ®?ïõí«r=?\§p2Ÿ9ï?UÖ$Yd–÷?\§p2Ÿ9ï?ïðw
S?b*{ªI'é?_ý±·ö?b*{ªI'é?ïüÓ¼ˆ»?&¡» ÷??Ábøº¤X?&¡» ÷?ïþÀþôxt?ŸGšÃž?#ðu–x×?ŸGšÃž?ïÚCi¥úÀ?~—®ùK?rÞK?"?~—®ùK?ïî¦Ö÷?nkAúƺ?aY)᫤/?nkAúƺ?ïñºgÊG?Nº—R•?\Šßž^ðé?Nº—R•AGN4FGL J2030.9-1621¿îÌiÊÀ=0]¥qÀ:®p¦[HüÀ<~b¼ºh@]µ%ç@…	Œ³?ÅÛï?z?£ö AÏ?à_‰gó.`@œ¤MQ¿ì0Ï«¤¿Ú6à;êfç¿åyÄ6%¿×'@~b¿×.ž
œ µ¿ïÿ"Év7AGNbcuNVSS J203048-162224?ïú¤oq¹??ƒA/Ύ?EnA-`"‰??ƒA/Ύ?ïêuZ'ÇM?kÄõn%ÕV?eŠ¥±½R?kÄõn%ÕV?ïâ7B6†O?dÇÝŸ/?mȽ~±Y?dÇÝŸ/?ïøÃâ(ºÅ?3Ë´59m?Lðv¾À"£?3Ë´59m?ïõª·#BO?OŒMŸ?Tª'oCѱ?OŒMŸ?ï
›bá;?—¦ûay?Lœ:Þ£?—¦ûay?ïÊ¥mQ+?}qË.Ev?zõ­[5be?}qË.Ev?ï߃H£?`¾¾q¶?Þ?pp¾S?F­?`¾¾q¶?ÞAGN4FGL J2030.9+1935?êW•âbÀ'
"cØ­À9¢^)ÊÀ;î=ÚV"L@å4!Å£?úpŸM7Á?·›þ£´{?Ä,ÞÅÈ¡š@°iS@/ÅÇ
â¿Ù4åOz'—¿ÚF0ÑY#ˆ¿ÖCÆ=çl5¿Ï;>š@¿äŒÄŸâ¿Þ|Û·Ì5AGNbll3FGL J2031.0+1937RX J2030.8+1935?ïõïÙ>?P—¾Ežn?T!È
F2?P—¾Ežn?ïŸPÁt»$?"küt҇?ˆ+ϛñÿ?"küt҇?ïÆ%‰…?}ù‰µË$h?|í;*A'Ù?}ù‰µË$h?ï¶*¬Úq¯?bïbþñÅÒ?'uTÃ4H`?bïbþñÅÒ?ï·ÆIGî?/ü'MM"?'mÇ|Øx?/ü'MM"?íUxúµ	Ú?À÷Ûï)™?µT8){Ê2?À÷Ûï)™?ï¡|3y¡?šÊu+;?Ÿ+Ðr±"Ú?šÊu+;?îž;×hÿj?R}6²?¦Bˆ""\?R}6²AGN4FGL J2031.1-2615?Úoh£Wˆ}À@G¦a(9À:‡îúôþDÀ<Â*²[1@ÀJˆdh@&†|†c?ÄZQDÁ%$?χ>.@bϾÔã?ù²jÉ!œˆ¿ïÿ"=ßßy?ïÿþ½à ¿¿Ü‹©_>¿çN(Ÿ~¶¿ãf[)òB¿äGGQÎ(íAGNbcuTXS 2028-264?ïE¯ú	¾? zpÏïï?—J?ú;? zpÏïï?ì!ÓjÜÓç?À½²Ï0æc?¾ñd©`Ç?À½²Ï0æc?î}"]«Še?™uK!4¯¿?¨-Ú#‹«?™uK!4¯¿?íCØ1å?—G>:ÊŒ?µá?
-¦\?—G>:ÊŒ?î{PÆl
•?§i5d?¨Jóœ®ò¨?§i5d?بSÚ!?Ñ0èØ=§?ãõ+Ör'ð?Ñ0èØ=§?ìjòœëË?¥i•Ÿ'ç¿?¼¨k§Á¥?¥i•Ÿ'ç¿?á%a2—N]?»&ý9é?ݵ=šÑcF?»&ý9éMIXED4FGL J2031.2-4121¿½øopƒÔ>ÀAÕ¥~ª*À;.¦Üx;À<³JÖ½ç@m·&tU@?e¦MC?ÎÖþÎ?à­]€ä–î@
¼{F@¿òRBm
¿îCšžý0Ã?ïÿÏù§÷*¿Ü/#" ¿æìÎÊÓοîCÐàWÄ¿ïÿ–ƒd£ïAGNbcuSUMSS J203056-411906?ïê™×µ'¥?oâüÚF¶?ef(rIÒg?oâüÚF¶?ïòýûÈä?cbУ©ºd?Z¿¾6¨ÿ?cbУ©ºd?ìˆÞtŸî?¥zÇmþ]?»¹|["?¥zÇmþ]?ïûzÖú'ñ?1¨!¶x?B£ý‡ÉÐ?1¨!¶x?ïóÚÇ{?gŒÈˆ?9?XJp¡[º{?gŒÈˆ?9?ïÓg?̖?"i§Í¹ƒ?vL`¥2´?"i§Í¹ƒ?éSìV³s"?±b˜¯"'?Ê°N¥21´?±b˜¯"'?ïìÖÅ?`DȦ1`?cüùó½?`DȦ1`AGN4FGL J2031.8+1619¿ï¶¥l`¦À+ÿŠ:›À:ºZ/ ~üÀ<?Ô|ñÃ@ó2Ûõ^¼@P³''d?É1Á¿"?½ä<Uäˆ?õ^yLò÷Ú@&¢¬ì?ïþÔI˜Ð¿å.)ÿ,ñP¿ìgß?–ÀÓD`,;¿í©¿Ãyè¿ïý›l°ÚAGNbcuMG1 J203139+1622?ïôÕP÷6?X½)þ‰O?WÒU`ÑD_?X½)þ‰O?ïÎyX9/ª?ØÈ&ò÷?xÃSƋs?ØÈ&ò÷?ïš8ïp÷Ë?‰å[·?‰qÄâÕF?‰å[·?ïØ3–Á‰3?\?ðr¦¶?sæ4µèÒ`?\?ðr¦¶?ïۗ©»‹î?y7ÿM˜Y?r4+,ˆÜù?y7ÿM˜Y?îÐÏÓèJ?ª PS:Ë¿?¢ó¿Ã'õ?ª PS:Ë¿?ïVÇEŠ‰í?"fÿ6®E?•'R^O?"fÿ6®E?ï	°KôX?%Iy'?žÉö…b<ý?%Iy'AGN4FGL J2032.0+1219?íq2ãAŸÀ/"š8ûÊÀ9ÃÁc>ÓÀ;ä"Àìĺ@)*Û£@ž®"i›?ÀCŸ¼ô<¨?Àìõ·&È?þ]†Þ«òb@Ç
ÈÀx¬¿±	[]ô§Ý¿åcØ·¼šP¿åʆÁ¥§D¿äG-»úír¿æ¬L#Å&¿ðAGNbll3FGL J2031.8+1223PKS 2029+121?ïûÑþB™5?;žK8:ŒÅ?@¸Ê,çÐ?;žK8:ŒÅ?ïيãüÇÅ?~Ÿ+ÙÄ?s:ú¼å?~Ÿ+ÙÄ?ïå­f˜¢?lÆþ®¨"Â?jRþml^µ?lÆþ®¨"Â?ïïÅ9sw?DíåЙªõ?`:Æøéà€?DíåЙªõ?ïè@	Ÿ)ë?e
<m]jX?g¿öL8lø?e
<m]jX?îރԓô?®øˆ‡ý?¢¹Ts??®øˆ‡ý?ïl½h´R
?'Šwu~ó€?'hRæ"½?'Šwu~ó€?﵆®Ÿ)?lú)ʧJ?'žTQ®xð?lú)ʧJAGN4FGL J2033.7+6308¿ç:ß²,¸@*øœýç!À;CÛ÷âûÀ<—έwœð@!'x´FÄ?ûÚ®‡ggî?Ì£J(î?Û@=²¾@ˑcj2¤@›KutK¿ïþ³™õßì¿í¯>;¤ò?ïÿÿ^ðP`¿§œÅ+	¿ßŽý'¬¿ì9Z'}rAGNbcu3FGL J2033.6+630987GB 203249.5+625814?ïðyà@Çñ?_ìûžJô?_?]sÝ¢?_ìûžJô?ïg}(Zù1? yRõlêi?"ZíÁ¡ç? yRõlêi?ï_пÂðw?‹Ù'xüÒ4?"è2U?‹Ù'xüÒ4?ïsªOR?‰
{.¡V?žñŠ¶¿õ?‰
{.¡V?ïã\¿¯¿?pNP|Õ?l£@~û©ž?pNP|Õ?îÌnœÚ†?¸»"äÞæ?®ƒ9»¬?¸»"äÞæ?î¨0–¦? OòÏÌÏ?¥|öõ»§? OòÏÌÏ?ëŸÃ^?±ŠåšÐ°š?Àéóš…Â?±ŠåšÐ°šAGN4FGL J2034.6+1154?íS_ތè±À0Œ¬¯öÓ1À9YiÂ;ySÀ;Žpð›@r¨h3@ÔdcP?½-—ÿÜÅ?Á¶—;?þi¾Å£à@k–JYÀf?ä"ÝÛ
¿ÝÆG·J/¿ægfÁ€Š¿èFl*˅¥¿è'áý¶z¿æXøŠ.ÃAGNfsrq3FGL J2034.3+1155TXS 2032+117?ïüÿŒMè?;ºÝdòÉù??@'2ª¸?;ºÝdòÉù?ïޟ±ûT?}î—qþúa?p°&÷W9I?}î—qþúa?ï×í2?e?pÂãLe">?t‰YÑÉ´?pÂãLe">?ïéÍ5tÎV?N7NjÛ?f2ʅ²J'?N7NjÛ?ïšwcþpø?‹ûWÛ¦]?‰b&üô%å?‹ûWÛ¦]?îý'$Ía??©Â¹¨¡­? &í²N?©Â¹¨¡­?îuÙtê§m?¢•ú"§g?¨¢h´Å%+?¢•ú"§g?ïšaødøu?tQLúµ¸f?‰gßâªå?tQLúµ¸fAGN4FGL J2034.8-4200?á« Ml3ÀB3´ÃÁ‹PÀ:C¿šµ"ŒÀ<a,"¹º@ W$"2LX?üsAü#Òm?Á¬ÐB£¿?ÁŒ÷Ÿ´:Û@ô즆çæ@db̨å'?ïþ6Ò$$¢¿ä杞6€¿ß¿YFÃ2ð¿ÎxÕäÎv¿â'jeÏg²¿äìf€<¦OAGNbll3FGL J2034.6-42022MASS J20345108-4200386?ïÿè{É?
¶í!=S?†îÝæÓ?
¶í!=S?ïôi]î?^Ëø¾çk?Wç-oP¥?^Ëø¾çk?ïï¹@¨ç•?kàîÚ÷Y?`F¿Lª¿?kàîÚ÷Y?ïõ‰J}7õ?9©‡àªÉ ?Tíjٕ§?9©‡àªÉ ?ïÿ]È'?[åÿö¶?Fðô`ú?[åÿö¶?ïÒ}äê¢?…GsÔZ'$?vÁ
›-÷??…GsÔZ'$?ï慐M?¤?s‰Œ˜²?izoï9{Ò?s‰Œ˜²?ïàTÈ\?ZZHÖrØ?o«nýêt#?ZZHÖrØAGN4FGL J2034.9-0450¿ï㷊p[ÞÀ91öº «À:tBúP"–À<N¿ïn¸D@T¢Ëò\S@b¥Z'"?Æ!Ô¦Šî±?Âþl©±?úÆqÔX²I@Mq6Ô¨¿êá:­z÷î?ïö'÷䨌¿äSÓâ?Ð¥¿äÈ'­ÄÊ¿ãÏ >ŽÛû¿ïø²<'ÎAGNbcuNVSS J203508-045029?ïú"LÂj7??‡'<'¼>?E®Ìä¨??‡'<'¼>?ïÏÎV\$?|"®Ž:ñ9?xÔƒÙ?|"®Ž:ñ9?ïÚHÉ"
?h'3ð"¤J?rۛâƧ?h'3ð"¤J?ïƼnþù?a$¹Ÿ}Ç?|¡Èw]››?a$¹Ÿ}Ç?ïË÷3u?~Z$g?zp"MˆC8?~Z$g?ï @<[%?¤én'?Ÿ[÷ÿSÓT?¤én'?ï.híž•?•lZØNò=?š2âZœ'm?•lZØNò=?îÑÎÛ´Šû?"%Ï6M]Æ?¢ãB#›N?"%Ï6M]ÆAGN4FGL J2035.4+1056?ڊQP\ôÀ1>F{åS¬À7²¼MùˆÀ;4Oó]Z@zø?kQ@".:¥î<?—³®e%0?¿¦Û ¢ŒÝ@"'o°'@}4JµZë¿Ë kÅËÑ¥¿â%¦V]Û¿å<Z#bØ¿æ£Pg  ‰¿ê$¯â±;¿èæÖcNƒòAGNfsrq3FGL J2035.3+1055PKS 2032+107?ïó.³4³?QAôœ¸?Y¢šM	zS?QAôœ¸?ïw*zÁ«ö?«r©Ý÷X?'°©'O8?«r©Ý÷X?ï̂gMìó?T•ö¼2?y¾Ìv–*h?T•ö¼2?ïûњfô?>5H€Í‹K?@¹•f3H?>5H€Í‹K?ï¬?ðʜ¶?Bõ¤ÛŒÆ?"ðÃ	þ§?Bõ¤ÛŒÆ?íŸÞÜY?Á#E‡ý¡?³O»?Á#E‡ý¡?ïwÈË^@?'é6 3¸O?'þísoë?'é6 3¸O?ïå§ûÝ?b×n)ëï!?jXúÁÌÆ?b×n)ëï!AGN4FGL J2035.9+4901?ӝ¾ÂH@ë@UZ¥À9‹'ªhô¶À;¸‹C•@ Ɋ8þyB?þŒÜò´½â?¼eáÜ(Šc?¼ØüŸ½?þ‰Às"6Œ@­¸ºÇË¿ïòö—¡qÕ?ïýŠuV¿âé>›A:¿ÒXÚaµÒŠ¿ã€¡{k¿Û‹ÃîúAGNbcu3FGL J2035.8+49022MASS J20355146+4901490?ïû¥ÁP^?@ß`aÓÁ¹?Ahú‰!‹;?@ß`aÓÁ¹?ïÓ*š}£?x¯L3·Hö?vj³múw?x¯L3·Hö?ïà6,ü|,?vÁAj¹ËS?oÉÒË*<•?vÁAj¹ËS?kՑ?mYæa܆"?‡Ÿe,`?mYæa܆"?ïð7Åán?\ۅ1?_Ð:ƒµ0?\ۅ1?î¦6‹Ðê?±ÀÎ^¬º‡?¥œŸsÓU`?±ÀÎ^¬º‡?ï— ¬?‹úÛ?D?Š9à̉?‹úÛ?D?î9ÌP¿ÏÓ?š‹˜½
=ð?¬c:÷ržË?š‹˜½
=ðAGN4FGL J2036.4+6553?ï¾¾Qè]«@-—µÐ1\À9ûžs.À<(Ød°ƒÁ@㬁u`?þº}>ïÿØ?¶_adsòì?ÃÅ£e@	Ê*[]@
,™­æƒ?ïþ;¤ñ¼p¿ÌcÂÈ&C¿Öë÷öFC¿Úå»d°¿çÃâB׿äLD琝rAGNbll3FGL J2036.4+655187GB 203539.4+654245?ïü¾¼‹-"?37ª^Œ?:
‰DQ?37ª^Œ?ï☀êÌ?n¸–zÑf?mg?ÏŠ?n¸–zÑf?ïå]s3åq?fÑ8¼fý€?j¢Œ¯=×9?fÑ8¼fý€?ï£6i¯­=?a®";\)?‡2e‰Åܱ?a®";\)?ïóYï4«®?TOLzÌ3Ô?YL!ÿÂç?TOLzÌ3Ô?ïVwÄ:_«? ec¸j}?•1zkØ ? ec¸j}?Aˆ-?‹
qBï[?Ž[/6O?‹
qBï[?îŸn—"¹?‰+ùëÚRH?¦	÷Pn?‰+ùëÚRHAGN4FGL J2036.9-3329¿ïxÁ†-è,ÀAśý÷èÀ:^x]ï"À<H™¤T(@!$/_>)?óŒïœÛmz?Ð.è¶7_?ÏÏ{¨Â×V?û'ÿ·@¨éÜ?Ž¨ºH棹¿è)!ACAH¿äLXÓÖ¬J¿ÃÃ7Îxt¿Ê/ÁŽ«)¿Ú&èa¨¼wAGNbll3FGL J2036.6-33251RXS J203650.9-332817?ïõõ
g_?QE›œrj?Tåµõòj?QE›œrj?ïà=õPpþ?~Ç5ð?oÂ
ƒ",?~Ç5ð?ï®·sZ´?'‡
Œ'€?"R#)£?'‡
Œ'€?ï÷: ã$}?:L'±!C?Q‹¾)8åý?:L'±!C?ïóÒLég¸?W~Ìû¥	0?X[fli_h?W~Ìû¥	0?ï4Ï@o‡?¤Ô-Q7y@?™n:A)?¤Ô-Q7y@?ï(ï¶ÂÛn?–.ô[o?šâ	"}(V?–.ô[o?ïê:œf±?Z
ãfæª?eÅc§
XU?Z
ãfæªAGN4FGL J2037.9-0504¿ïéÙÊ®†ÞÀ9ñD»ó¡À:ý]0\¿À<‹;Óåj@ J@–H+?ûGã>(Y»?Ô2本ž"?Ìÿ9[–S¿?ûTâæÅ°?ý?]Rìa?ãc	¼Ad¿ëI‡î'ð¿Ï1~¨&¥¿Ü&š¢þ¿Óôk0Ñ¿ïü>àŸ°AGNbcuPMN J2037-0508?ïðq¶6ïg?Y5|"`39?_""bÂñ?Y5|"`39?ïËáz#™?5Ôå-?z}&ÁgÃ?5Ôå-?ï£HzÔBÉ?ƒõ¹*…œ?‡-á@ yË?ƒõ¹*…œ?ïÈZn$d¨?]²z4PI?{ÒÈñí3ó?]²z4PI?ïå•áSAœ?hG~^Ÿ±'?jj!ü«?hG~^Ÿ±'?îÖnåC™»?§]Šlýo²?¢™§záP?§]Šlýo²?ï6c/pÓ?"£åWE&Ê?™3žôê{ž?"£åWE&Ê?ïh9¿N?‹
ÛF×?ž2øж¼??‹
ÛF×AGN4FGL J2038.7+5117?å"`þú
@ÿA<á1ßÀ9g{o'VÀ;A_ˆü"d@¦ºZ•@Ó}c-Ø?ÀúX R…ß?Ó±Zÿ@¾6`]'@ˆ"ŽJ[¿â°¿?ñ\¤¿Ûò–Šñ`*¿äÀ~«Ê*¿èÝ_ìú•¿î¿ñQçSa¿ïÿW-ä>ÙAGNfsrq3FGL J2038.8+51133C 418?íóÒ¿ÍW?ªÄž<,`?°gál'VÂ?ªÄž<,`?ïƺ.î¹?†ÕŸcšõˆ?|¢è–º"¦?†ÕŸcšõˆ?ëšKo?ª†ÒK³á?ÿ'–ÑúD?ª†ÒK³á?ïÎþâüË?`š.›¨‹?x€n¶^?`š.›¨‹?íó&—ˆ6?­x4|©?³€fÉùãÐ?­x4|©?îpBGD¯?±÷80äs?¨ûۋµ?±÷80äs?å¯B´k¾%?³s=?t¶Á?Ô¡z—(ƒµ?³s=?t¶Á?îd¡Vì?–Ú]U±èd?©¾åê'??–Ú]U±èdAGN4FGL J2039.0-1046¿çzPœ¶À­À<¼{՝VÀ8¹
…"ÿ×À;°¿òɶ˜@´VØ~ܪ?ÿK Íj~?¦I³RR]E?·Ûþ2¡N@÷•p?-<@ٔ媿1¿Õ§D}"¿×ÖÈ#DӚ¿á8ãv\~¿àÓ> L%È¿ã¾XˆWR¿èM3>ñ­WAGNbll3FGL J2039.0-1047TXS 2036-109?ïù¡M†àH?I:vˆ]А?IzÊVØDº?I:vˆ]А?ï°eCYN®?'C²DPàð?ƒæ¯%ŒÌk?'C²DPàð?ïÅÈ£¿¯¥?èìŸ?}®»ƒ?èìŸ?ï¡C]Þ?ixH¦¸í?‡¯9̦ø'?ixH¦¸í?ïâ†Oà2?në7¥ïwv?my°uŸ-ž?në7¥ïwv?íÇ¿q;ùÎ?¹Û—''Ë/?±Âvü'?¹Û—''Ë/?ï"þ^/N?1¢Ô¶ú?ŠÀhqu¼"?1¢Ô¶ú?íî«ÅHҊ?–µ
} Uû?°Š¡Ö'_-?–µ
} UûAGN4FGL J2039.3+2150¿çÍÉ)wÀ'©K{(•JÀ:"Ï$•á~À<CN"¸‰@z…Nˆú@ºòDUšf?Í»Ûۈ|?хRdÑ»Ê@ø¸BÒ¨@'ہÆi?ïÿEÅÜèìêÿ½ºá¿áiž)KS¿ë¶
éh¿ïö¦…:g¿ì8ÄL0ZAGNbcuTXS 2037+216?ïï± ˜Þ«?tÐ~ï‡k?`N_Nd%?tÐ~ï‡k?ïœëoòx¥?Š·ORœ±±?ˆÅ#ÿò:±?Š·ORœ±±?ïQ•T̜7?‰àúÀËë?•ÍU_A7?‰àúÀËë?ï6>
Š_È?w.û'–uå?™8>IŒœù?w.û'–uå?ïÎ9›¤ƒ$?xgÓò…–÷?xã2/Eü?xgÓò…–÷?ìç+Q@Ì?¿·[Š"?¸Æ¥qÐ8"?¿·[Š"?í"
™ƒl?£½V îÄ?³d©ê
%?£½V îÄ?ëy"o…c?¤Ê¢šÝ?êvAêu?¤Ê¢šÝAGN4FGL J2039.5+5218¿Ãà¦Ñîþ.@[]ô§ÝÀ9èê1ÄÀ<Þ7X@!ž†)þ?üÃPíX]?¹&+¸À{[?¨ˆÝ³N÷?ðcª2n?þ!M:ƒ?ït²ÄãÊ?¿ïüáù?ïöóçÃɿ丕k7¿Øædÿ´¿Ô…qÄhzAGNbll3FGL J2039.5+52171ES 2037+521?ïùP¨±[ú?A<ÿsŒð?J½]^ØÂÊ?A<ÿsŒð?ïÖz¶o?{½%öðÈç?tøB Ô@s?{½%öðÈç?ï֏<Y³·?u°çÈ2 ?t¸aÌFì®?u°çÈ2 ?îüw˜E4?ŒÍs0'QÓ? 8†yï>Ä?ŒÍs0'QÓ?ïé̸]‡£?aϮlj-?f3GÄÔt¦?aϮlj-?ï9V'\™?¤:Ô·-Òl?˜ÎAó¤Ú?¤:Ô·-Òl?ï·Kîëۆ?…Kû(`Þ?'-=yú—?…Kû(`Þ?í£Œ'jÃe?¨DD"zÆs?²ã›t;ñ[?¨DD"zÆsAGN4FGL J2040.0-5737?î‡z‰DHÀB‡DÃ~orÀ:+jî‹cvÀ<K¥"cØ@mdõxµ@ÉÚª"?ºYF¾U?¢Ì~HZaË?è¢FçE?õ´k×êb4?ï˜Úϐ¿áƒ]©~i¿æJÀ¾¡'¿à¶}Õî´~¿éâ…0V	!¿ïôÚgÀºAGNbcu3FGL J2040.0-5734PKS 2036-577?ï처£.?^ëöÑ2®?cMh·ª3?^ëöÑ2®?ﳫ¦a~?Ž""æb'?ƒrGB!?Ž""æb'?ïk‡4ð«?¼–ž½oã?'ž/¸˜?¼–ž½oã?ïFׇ]N\?M"L 	?—%žf~?M"L 	?ï…|þG2?†Ùj%Hõù?Ž Àx'R?†Ùj%Hõù?îøSÈBé#?¬àÔ8u(? zÀðÒ?¬àÔ8u(?ï,¹Ïø"?"ÜfU›ÿ*?œZh'Sˆ?"ÜfU›ÿ*?ë 84­dZ?ªšð<Û«÷?Á-Jn—?ªšð<Û«÷AGN4FGL J2040.1-4621¿ÓñiBþq#ÀBкs-õÀ:¶€À<p.½'¬î@ øŠ/nW¡?ùâؼ²£?Å®_¹Îî:?Á¬;ç%?ýõÇèa}É?þ1ÿ§?êØ+ÛPO¿ï痞—°5?îõ«þO¿Ù˜*™0¾¿à/ ×{|x¿Çyœ#6»ÔAGNbcu2MASS J20400660-4620180?ïþb	ú¤? ÛÔ%
²?)ß]	=(^? ÛÔ%
²?ïít7½å?e¹)_}q£?b‹È¡ÚM?e¹)_}q£?ïîåõN"?`ys Áð?a
ž»«¶?`ys Áð?ïÔíßÛ·?d4Ü㓶G?uþ‰1¾PJ?d4Ü㓶G?ïû¡ÒUÖT?@[eœVL?Axµá£·Ü?@[eœVL?ïºÉà3[ø?œË錛æB?M‡ö@§þ?œË錛æB?ïé_—6µ@?o]aÙ.?f hïÆ_•?o]aÙ.?ï'*Ë8Uº?ƒ+ùŸêô²?‹µM8ÉÉX?ƒ+ùŸêô²AGN4FGL J2040.2-7115¿ìøP@µ&éÀAs–Б}À9èFžÀ<<é•Zo¸@!Ž^I·?úIޚTª?¶UˆÞ
ŒÌ?¬_‡œcoÞ?÷ƒmjW@H­Ù©T?ï§hß½jY¿ÛÄþø*¿Ô;ýÊ
ü¿Ú&æô–?r¿Ô=¡ K¤ï¿Ñ*=áb.AGNbll3FGL J2040.2-7115PKS 2035-714?ïûÙüFs=?4OàJ}†¤?@˜6ÓÉB?4OàJ}†¤?ïñº·˜Õq?\1…æ‹É"?\ŠN¨?\1…æ‹É"?ïèçKÑ?c/2Ô-á/?gñæž?c/2Ô-á/?ïã<8H#Ž?S×ۓ£@?lÃǬݲ8?S×ۓ£@?ïô+›ÌÀ?M•¹`²Ù[?W¨Éü¥ì?M•¹`²Ù[?ïÊ`ùaw·?·©£÷œQ?zσUsp®?·©£÷œQ?ïÜü`ÊVa?{á}9åʍ?qÏ«Rï[?{á}9åʍ?ï¦ÂÅ<‹?sÕ÷º×lç?†O_"b	f?sÕ÷º×lçAGN4FGL J2040.2-2506?äN¨h©žÀA4'¾‹ÁÀ:³íضÀ<i"`šu@qàqo@àú)&j?ÈQe£Gî+?ÂOÒ:Ê×)?ñÝ t-Þ@7 ¼c?y¿æ*#õ¨Ž)¿å4¢žûÙ¿çe-BŠ¿¿ïÿËý™ô2?ïý1¹¶o"AGNfsrqPKS 2037-253?ïÙ"Ø5ûS?p:¥›ÅÐ?sn"Ú³']?p:¥›ÅÐ?ïÐÀl—-?ƒùðˆÊ¬?wŸÉËê?ƒùðˆÊ¬?ïO×dß?Œœš±Æ?–{?Œœš±Æ?ï¦-½Â1­?qÎpšá?†t~EˆÔ?qÎpšá?ï '°¸´?û:¿ÉJ?«ï©èé…?û:¿ÉJ?îk´›•Œ?±±&î2Kw?©D¾jÀA?±±&î2Kw?Jâ|a?à|ƾڋ?§w‹OD"ì?à|ƾڋ?ít¹>¿GB?£ÛÚ(Lr?´Z6
s¹p?£ÛÚ(LrAGN4FGL J2040.5-1705¿ì Áè("À?—‰Åæÿ~À9ÇlÝxì{À<.œ×%@™ø÷øõ@l—E+ƒ<?±úëC/Ÿ¿›V)úœ¶&?åçÐ^QÅ@˜gu/,?ÝZr§½HË¿åǞ¢ŸÓ¿è¢ƒý†(¿ãδ˜ù`ª¿â~5ZTà,¿ïÿ»lR8²AGNbcuTXS 2037-172?ïý³‹¡øý?'&ú Sf	?2c¤ÂixV?'&ú Sf	?ïìï¯Z ?h`€nˆrx?cPÊè¯ù?h`€nˆrx?ïëêT6í?S¸%¨µ†)?d«ñ‡'›?S¸%¨µ†)?ïþ¤"?{|?òI6¾š?%·¾Z¹'?òI6¾š?ïýÝÄtlA?3žßc»¯?1Þ,œgŒ?3žßc»¯?ï•zÆÎ8»?".Îà?Š¡NVÀ¥#?".Îà?ïÓvCË~;?z¡¶ž5(b?vDÞ҆Ì?z¡¶ž5(b?ïüxÅÏò?-z_dºúÈ?<?™±¨?-z_dºúÈAGN4FGL J2041.8-7319?î¨áfÀ@ÜL˜_À:¯UQk,ŸÀ<•íÒt@ ò¾Íە'?û0íÕ·?È''·ÿá?»Q'ľ5…?ôÓæIîa?ù§zÓZÛn?ïÜCb¿æD¼'Âåÿäµ&Rz X¿É]F,4;q¿à•t;;?q¿Ù^¡IòAGNbll3FGL J2041.9-7318SUMSS J204201-731911?ïþKèêB\?2S2r(?+AnO?2S2r(?ïçíÖ÷aæ?n?Ä°°vÕ?h(ôr‹?n?Ä°°vÕ?ïñô§ºÍ$?a·IŒÌ»µ?\°òÙØJ?a·IŒÌ»µ?ï×4ð!»'?VÙûïtÚ?te‡Ü"SQ?VÙûïtÚ?ïþ5ê6ƒä?!÷(Sîã?,¡^Qª'?!÷(Sîã?ï´
«w	?‡Ûí7a§K?'ýUÎñ?‡Ûí7a§K?ïô¢
}äT?`DPÄÃé?V»å4ØO?`DPÄÃé?ï=ü±';?/èû¢è?˜@iÜÐkŒ?/èû¢èAGN4FGL J2041.9-3735?·X±÷"O¥ÀBž FÇd®À:qíâÇ
À<j+…¿È@ ÛB±Ux?ÿŠ7/+?»A*—®2¿~À!´(é?ÃG¥NX©@‰}G(ˆŠ¿íÖ±v/?áµü`äs¿ášmÔﱿÛSJÕù¿äh¸@"ÚË¿Àr€óZ€AGNbll3FGL J2041.7-3732NVSS J204150-373341?îQäAf/g?Å-ªPs?ªá»í茂?Å-ªPs?ïæN%|ç1?s+ï$!??i±Ú"x¦¬?s+ï$!??ï>g©Sî6?™Ø³øÏæÜ?˜3
ҝA?™Ø³øÏæÜ?ïðò€‡ò?E\¦˜C?^þÉ "Å?E\¦˜C?ïÃL3Æg>?…^˜6¤0?~YæmÈõ?…^˜6¤0?ï/Æ`?¨*{ÒÔæ±?š?~3üK?¨*{ÒÔæ±?ï5V™ÈF3?›P¦ÆÙ?™U,ȯŸ?›P¦ÆÙ?ï΃Å9Q?jö»Ôô
ï?x¾uDoX?jö»Ôô
ïAGN4FGL J2042.1+2427?Íå¡ÅbZÀ%'Ó"wÀ9åÚ rfOÀ<$;¿É¯@ y2&ì±?þa8"œ×?´›m"<æ?'vx_ë¬?àØ¢mþ‹@JÝîZ¿èœf2d[?ïÿ8Yã¡%¿ã7; ¿þˆ¿Ô|_Ìï1|¿ågðßьO¿£a+'AGNbll3FGL J2042.1+2428MG2 J204208+2426?ïý—vîb¸?*²Þ¬ØtU?3DHn ï°?*²Þ¬ØtU?ïäeù6Àº?tEÀ'Ð|X?kš»€Ö?tEÀ'Ð|X?ïôN…ì`?IçC5³—¯?Wbôõ š?IçC5³—¯?ïç­°Å?TJ¶îý@ã?hRçCž¢Ü?TJ¶îý@ã?ïúr?Sõ?@æÔ4–U?F7§?)J¤?@æÔ4–U?ïRÉ\ïˆþ?¨lóÕn?•¦Ô\çvA?¨lóÕn?ïê4ëU_>?p¶Ãù¤ÿ!?eË€š?p¶Ãù¤ÿ!?ﺇ!¿9ß?w}I"²"÷?^7•üT?w}I"²"÷AGN4FGL J2042.6+1629¿ž<{"˜À/*Îî<´À:Ä_½Õ¹À<]JÛÆdÔ@ ü›nÛÕÔ?ûC«Ë]a?Úù#¢œwš?ÈÜ!>6?÷€¬¹1@[K€1È¿ïøŽß#?ïÿt¿Å}M¿èJR]¿ª†ÁáÈm©¿êU8Á'‡?¹%ü"äÎÌAGNbcuNVSS J204242+162910?ïû¹âdc­?V'°åã?Av³¶96?V'°åã?ïÖKª‰'?'æý$Vj&?týZ"|&û?'æý$Vj&?ï²GZ²~?€õf]ÿÒð?ƒn)Zïž4?€õf]ÿÒð?ïìà$\D"?L¤?`ók?cÛ¦{µ?L¤?`ók?ïú%=¯Á'?KYÈL1Ýà?Gk	ŠÞ?KYÈL1Ýà?ïBË_B
?¤òå$æ?—¦ŽðTY?¤òå$æ?ïbÈK«š?Ž–§[U›?"¦öŠœŒÏ?Ž–§[U›?ï±~f§l?zëOUâº?ƒ f"œÆð?zëOUâºAGN4FGL J2042.7-5415¿ÏŽ6ë_ÆÀBä›A9†4À;G™Ò¤}"À=<ßP]¦@H;®@€"d®ÖB?Ñãz¥vÈ?ïÿûB«÷@FøðAF?÷'ïUÑ?í#Þ¬s;¿ˆÛ^¿‰¿Á–½FG.¿ëŒ#>Éik¿ïÿó€?ÖZ?î€Ý`í²AGNbcu3FGL J2042.3-5416WISEA J204241.98-540925.3?ÝyŸm±g?ÔxƒY'@Û?áC0?I'M?ÔxƒY'@Û?ãöÆ~æ A?Î[ò©-<?Øs3¿~?Î[ò©-<?á0QŽ_v*?³>¯€E;?ݟ\ãA­?³>¯€E;?Õå%¡Øµí?¸¾-ë©9}?å
m/¥
?¸¾-ë©9}?Õ «3þgØ?ÓîÐá7§?å/ªfÌ?ÓîÐá7§?ƇÔ,4ç?Ê×»­ˆ?ê^
ôòþ?Ê×»­ˆ?ÆzE҃VG?´¸b:¨_•?êan‹_*n?´¸b:¨_•?£k9]~<?™r¦û&Þ?îÉO̓cl?™r¦û&ÞMIXED4FGL J2042.7-0155?é›8ýUÀ9iÂ;ySÀ:¶ãÊ?SÓÀ<_Öñý3@Ð3Xœú!@I:÷LÓ?ÇÐÜ&$?·vi¾µ‡â?ï:"£§@'èYp3Å?îò«ž~Û¨¿ê'ÇÅüÏ¿Ø̟ëÃ2¿ê3oce*&¿×'~!îè+¿èM?£ÙäAGNbcuPMN J2042-0148?ïøSžì|?KSCÒ)ùú?N±"yâÙ¶?KSCÒ)ùú?ïß*Md…?oWlØVQö?pjÙ:‰?oWlØVQö?ï¸
ZCdÑ?ƒŸ:Yvv?ýid×÷Ì?ƒŸ:Yvv?ïãuÜ-Æj?Q~è?lŠ#ô•­k?Q~è?ïâp"fEs?i •+¶À.?m{дLž?i •+¶À.?ïF,¤ùŸ?ŸüŠ"dz/?—:kd;¹¡?ŸüŠ"dz/?ïPUCB9?"ãæáˆ?•ÿU^vðÝ?"ãæáˆ?ïZðTÍrö?'áM<:Å+?"¡õ_riE?'áM<:Å+AGN4FGL J2043.7+0000¿ëãk´À8Â:îéWÀ:oÒ0¹Ü/À<\g=
¨@zî(½
'@n[þ-˜?¾¬ƒ×œ?›ñ"F7`®?àU'"W:@§6ycÄ ?î¹Ú¡÷Œ¿½Î6YX`ê¿é킺Z'¿Ý§]CýÜ¿Ú«zl­¨D¿ðAGNbll3FGL J2043.6+00012MASS J20434215+0001193?ïø™|ÆØ ?Uµ¶áÄz?Mš
ÆàU?Uµ¶áÄz?ïæç½`j›?m•Í-,y?iBŒW"Ï?m•Í-,y?ïڋψ¿?u{qÁ¡"?rº¹çÌf?u{qÁ¡"?ïõS»©í?<þÀ›"+?UYøî`"Ä?<þÀ›"+?ïÈò³Í]¨?~\$ÚZ?{†¦˜W?~\$ÚZ?ïìÓí]?—›©qÜnß?eyÆ.g?—›©qÜnß?ï•ÌÔj·?Œ™hÎûV?ŠŒÊÛg?Œ™hÎûV?ïר×`_Í?aÏÚ@yR?t+"Aa½i?aÏÚ@yRAGN4FGL J2044.0+1036?ïQeәo¨À30%"ôÇÀ:Ìóf"‰À<UcV­Í@8[ƒˆ?曥BDH.?Û`ØóK¼—?ïÿۂr5¨@‰
]Qï@
ÊMó(O¿í.Ýãö_?íSq+¼Fm¿æY©ŸK4\?­(<	E£ù¿ïÿÏ=ÀTï?Җ'ýCDAGNbcu3FGL J2044.0+1035NVSS J204351+103406?ïÓŽ
I?…Û=œ«7?vpxĨ;?…Û=œ«7?ïÓ¢:'<?rÐáë&.?v.ñ…ùØ?rÐáë&.?îזŒ?Ÿ"7E8.Ë?¯¿¢ƒ'[F?Ÿ"7E8.Ë?ïó~ñ]áï?MÓXR¥û?YO:â"?MÓXR¥û?ï¹ÚÌê©×?'†×¦î·?‰L½np+?'†×¦î·?îœAûoo?°ïf"öYv?¦?»àI	?°ïf"öYv?îLªÙïm?Ÿ×…Ž8¬?«5Raë.?Ÿ×…Ž8¬?ïñAìçýÞ?csrtƒãä?]|&'ùì?csrtƒãäAGN4FGL J2045.1-2346¿îa)¢ÞVÀAm_Eà´áÀ:‰ =!É~À<|µwE²@•òôÿ›×?þéùc-ÌÂ?ÂÉë›ïà"?¶]΁¸1?õ`Ɋ"?ü˜k&ºó¿ïÚÍáŸÂ©?ïûû…Fü¿âµQñd[Ê¿Üè˜DÚÐq¿æX²é̷Կԙ}_QIIAGNbcuNVSS J204457-234643?ïú7Eð?=:d8ߞÈ?G#ƒ|â*?=:d8ߞÈ?ï¶pøÄ*?'pãæñpƒ?'cÁÇ_¨?'pãæñpƒ?ïØÀ'ç.ß?uƒÅ¾ÛÞf?sŸ·,øY?uƒÅ¾ÛÞf?ï"×姵?s#؟ƒ[q?ŽÊ§lž—?s#؟ƒ[q?ï­Y?X€ÑÚ§N?a\ê—.'?X€ÑÚ§N?î€içq¶?±&WŽ¤v?§ùa‡,Ð0?±&WŽ¤v?ïÐÍúì'1?~PmdâÅ?w™†GKQ?~PmdâÅ?í|ÕG^}(?¢ÂH€Ë?´UÆÃäÀ?¢ÂH€ËAGN4FGL J2046.6-1012?ä…ÌþÔdyÀ>1Î_pÀ:ÀÛÉ¿ÒÀ<sÏÃøõ@ 33Yæ?þ†ÃÓÿÆõ?Å!#ü‰}î?³Žç á?ëjÑ?MGÜ?ý¸]ϓüw¿àDÝ¢x?ïøðâUË¿âó[Ao6¿ÜD""†ã¿Úþ;¤ñ¼p¿åa8^ì¢AGNbll3FGL J2046.7-1011PMN J2046-1010?ïûá°½*K?7•<ˆ?@y<ۂª~?7•<ˆ?ïÚup*Ǝ?v(w
Ø?rÅGÿ:`¹?v(w
Ø?ïäp
»+ ?jñþ€ë8?kõ=õ¨?jñþ€ë8?ïÑ˲™ß?]™ $É3?w&éÄp?]™ $É3?ï󣪃e"?S®¹"[?X¸«1ì?S®¹"[?ï1µÉóK?¡Sø²?™ÉF¾'þ?¡Sø²?ïÚ9v»•?{§jYät?rãD™F<l?{§jYät?ï.pÖ#Z?ˆ–8 ð?š1å6mRÓ?ˆ–8 ðAGN4FGL J2046.8-4258?ïþ@Vv,ÀCXœM©?À:Ö0Ï«¤^À<"üæp@>M(|ËÙ?þ>O%ØÝ?Ï]JˆåAc?њýôþ@:'FK@
ٝëØ¿î·3"Hø?ïý̞ÿŠ¿ß;!`Lò¿á9ýñ7¿ê]ß3á¿ØâÏØðÇ~AGNbll3FGL J2046.7-42592MASS J20464397-4257134?ïþûÁ£?$2Ñq%©´? Cò/
´œ?$2Ñq%©´?ïô÷¦j7?`=[袃?V³sÝ?`=[袃?ï—i´W=²?ƒ§_:8è?Š%'ãQ[ƒ?ƒ§_:8è?ïù›]¥2æ?5yœ]Žé?I'ˆÉ"•O?5yœ]Žé?ïþØм£?&p²ÏQ­Ü?"r÷¥%ÿ'?&p²ÏQ­Ü?ïÑC´	Ý?"ß'-?wu^,Ýo?"ß'-?îèàŠ€]?–¼þ±G÷k?¡q÷UkÕ,?–¼þ±G÷k?ïèº&‰?ZÖ_"_\?gEÙóå·?ZÖ_"_\AGN4FGL J2047.1-7400?éæÇâï#À@ì4~ŒÍÙÀ:ê»±òUóÀ<\{Xeò£@‰)Ô½\@Ü0ûJŽš?Íb@<??ªzK[Ú,˜?Ù0ù½EÆ3?ø¸+Ë	ÿ¿ïhšˆ¬âL?ã"×/Û¿ë΅¿G(3¿ÕµÔl©¿ïcȑԩ:¿í¾ÎaÍOAGNfsrqPKS 2041-741?ïúm_\?EÜú‡û³?FJ€í[Û?EÜú‡û³?ïÍ>w4?Š[M±ù1¼?y`ÄM8ÎA?Š[M±ù1¼?ïfܒp8?ˆök©1Â9?"<DjB]?ˆök©1Â9?ïØÕ.›?\ˆÎW@?sô•Š^œÒ?\ˆÎW@?ïó_¿òã|?\dY—0–?Y@€›jWù?\dY—0–?ïB;™‰(ˆ?¦×~žÄæI?—¸ŒÍ# ü?¦×~žÄæI?ïGBÅނ?•0€î€ef?£Ô"½?•0€î€ef?î^ÌÁ0®Á?Ÿ"—]²Á?ª3î¬áï?Ÿ"—]²ÁAGN4FGL J2047.9-3122?ï`ýMjŽaÀB±" ³Ô®À:bý%Z-À<køIRYi@jñõ%["?ÿô½±§?Äݑ€›pß?¿2&˜Æ
?úMn³<@&lXÁ?ïüšà–ƒ:¿è"@¡°¿Ü$.³q±ô¿Þ$)ªô4ñ¿áq¸¿y¨
¿æ^Ê@*'{AGNbcu3FGL J2047.9-3119NVSS J204806-312016?ïýy—½î°?GJQe:p?43D N}´?GJQe:p?ïáÜДÇ<?t] 
ãج?n#/-_Ì©?t] 
ãج?ïÜáTÄ'?v¶ˆ
¥žS?qUŒA½?v¶ˆ
¥žS?ïéoÏ_'ü?G/ÇKҁ}?f0Ї‹]?G/ÇKҁ}?ïõíù©_ñ?SbPCB¬™?T$ú7\Ä?SbPCB¬™?ïpL|Á'Ó?–ÉÑ«êæ$?'öp`ðm¬?–ÉÑ«êæ$?ï¸=1€þ?ˆ%
Œ²Å?ð³¯¸öq?ˆ%
Œ²Å?ï°[Ǟ\?oÅ.HîÖ?ƒé#ÃÒ?oÅ.HîÖAGN4FGL J2048.6-6804?ïÒ2t=áÚÀAì¹w…r›À:FNEÞ1À<w3Ï:eW@[9ë3?H@êùÞ}Ï?ºÃ¢Ÿ¨?¥4V@Jë-?ìŸóOîU@'Le¿ïü">`¸Ò?ïú³ääò¿èbªºSM…¿Êå9ñ=o¿åãflE£x¿ê.ՀzŽ¼AGNbll3FGL J2049.0-6801PKS 2043-682?ïü­!ƒ)ã?.]¸8müº?:–ôöE:?.]¸8müº?ïóȏ%w^?Y+{!•I?Xná9_T÷?Y+{!•I?ïïGǦš?]8_ó?`¸84ážj?]8_ó?ïòNó>aÌ?E'ÅQDÌ|?[bö¯Gù?E'ÅQDÌ|?ïùW?Š?D¾gÊk«?J£«¦Ž¤?D¾gÊk«?ïÑ3"šaž?€îÃõÜe?wf=Å]Í?€îÃõÜe?ï漂ÛD½?uHLbjÁ‡?iC}P¶Bq?uHLbjÁ‡?ïÇÙI3?r?ï÷L½?|[`¨©-?r?ï÷L½AGN4FGL J2049.0+1647?í­vµïÀ0¦ˆŸsÀ:¦ÖŽín-À<C瀭9Š@,»h zÊ@¬Å@'H?ß;Äý ?—ñ`CÑTá?Øó÷ÿ*˜@	è	ê§?îÐvoÈå·?ï˜þý–ï¿ãÿ‹Á>Ï¿çWÌ'ãt¿ÖâénÄú¿ßq+{ÙÀ%AGNbcuNVSS J204902+164727?ïüÒ´ äš?2~ÛDöÄô?9jX÷b^a?2~ÛDöÄô?ïÝ&f¥ì?{ò÷ÚÇ?qlÌ௉ñ?{ò÷ÚÇ?ïî;˙W;?[M
@,°U?aÄ49Mí‰?[M
@,°U?ïì UŠ÷?KÇ÷ÆÈ?cùߊءB?KÇ÷ÆÈ?ïòùÜUŒ?Wqý¾EAF?ZG¸X¨	?Wqý¾EAF?ïr=ÆEZ?¬4ÛlâQO?žñ¸@X½?¬4ÛlâQO?ïېñºÔ?xWU
mG?r7õq%?xWU
mG?ï¬v¿`8á?vS
þ°#?"âP$'+Ä?vS
þ°#AGN4FGL J2049.7-0036¿îט[)ƒÀ:`Æ÷ µîÀ;ŕ$¿ÒéÀ<³YÿOÖØ@#­ieIZè?ø–þ–µº?ɺˆç𔨿¥L9iƒ&f?Üi•ûg¿@ßÇÓ顚?çFyáîG¿ïÿþøþ"?ïÿÿ²}@?Ä/Mu~²8¿ïþø?ïñ"b"4AGNbll1RXS J204921.6-003930?ïï81DÝ?pÂ~uìã8?`ÇÎô¹â¥?pÂ~uìã8?ïàÆÇؤÐ?€ö·t#}?o98^ðM?€ö·t#}?ï<¸_­d¨?ŽŽ€Ù%Ã?˜hôãÏ?ŽŽ€Ù%Ã?ïâf¦kþÆ?b¶L72?m™Y»Ü²B?b¶L72?ïï§@(í"?a>â kV?`X¿¤85©?a>â kV?ï{Š¼uÖ`?—bø÷àj?Ž¨h®.?—bø÷àj?ï—ÅyÏØN?ŠŒv¥¶£å?Š¡yˆ—?ŠŒv¥¶£å?k¸t??€ùîx®?€í—w?€ùîx®AGN4FGL J2049.9+1002?ó<À4µt'yèÀ9FÛeNÀ;×/(·Ä@ÙƐȐ@'£}H*;?±âò~Jf?¸)ÙBQ@
£ì¤©(@h©ÿ˜Q?ïøkK¨tÿ¿á­#ŸAyG¿æÚw_²íþ¿çL£FÁ…q¿ëC®á){$¿ïþh@0FÅAGNbll3FGL J2049.7+1002PKS 2047+098?ïÏöhZ:?­ž"iÔ»÷?x˺%Ǻ?­ž"iÔ»÷?ïāCƒÚ¸?Ê¥Ã-¹?}¿^)tü(?Ê¥Ã-¹?ï"~?†ëeˆ½K?Žù qMjÚ?†ëeˆ½K?ïÏ:VNQƒ?]ŸJ«›_?xbÔòDZj?]ŸJ«›_?ïŽAX(ÏÇ?ñqD?Œo©è
žc?ñqD?îJ­ØbN¡?¶r²"à&\?«U"{'ãì?¶r²"à&\?î>y6fˆ9? `ñ®ïÇB?¬l–'àt? `ñ®ïÇB?ï
Aö"9C?ƒœ
é?ž·Á3!ѝ?ƒœ
éAGN4FGL J2049.9-2453¿ÕYË8ÀB¶â—À:úÎû{6À<_ü@WÞä@´wWû>¥@nxžwNì?ÚÅ>c?â öàqšL?ïH'AÖ@xh"<]¿ïO>â=ø3?Ô_ÀÚÑh¿ÓñS)rÀ¿é{'¾Šêª¿ë{H`A^?ºdÈA!ÞLAGNbcuCRATES J205011.52-244811.6?ïô%¬
?\Ÿ×W•±?WÕ´ÃdÅÝ?\Ÿ×W•±?ïçå›7?xT ™·è?hñÞ(8´?xT ™·è?îe¤+ئ?–5
lÎ?©¥½L"Ù¤?–5
lÎ?ïãb+:¹?V܊fj'?lôá#ß??V܊fj'?ïÕáù&>{?|੅@bn?uT#'ß?|੅@bn?ïŒ`Ëò²:?'
–Þ?ŒçÍ
2©Ž?'
–Þ?í·Ù2S? wGɾ§?²A6mǦ? wGɾ§?ï–÷!xå^?|ÚK^LåU?ŠB7¬||?|ÚK^LåUAGN4FGL J2050.0+0408?ۜ™Ïۆ4À7ùb¿ù'À9r{'pÖ,À< ¢ûB+@\Ø%ñVD@BÌ}òt&?­I¦èÃ?qßKäâ?ÅóH6¥ƒˆ@P5Þß?Æ{Pða§¿ãOÅx¿å›Èé}±¿äb\¶º;Ñ¿Ü]/ñ_SM¿ëçZ¢bëÞAGNbll3FGL J2050.2+0409PKS 2047+039?ïú(¢WûŒ?<ø.VÁÀ?G]w,Μ8?<ø.VÁÀ?ïæj@QŽ?pÓEs"÷?i•¿²Š0?pÓEs"÷?ïêÈ&b?m
.¸ÀGy?eí8"n?m
.¸ÀGy?ïðå÷žÌ?KíÃFò<?^5ç‡R$?KíÃFò<?ïæzÃj£b?b¶Ã=Zh&?i…<Ý>?b¶Ã=Zh&?ïv€t{õ;?™Ðƒ7Bçz?'/ñpX–?™Ðƒ7Bçz?ï±ÇNøOv?†Ìdz!Cá?ƒŽ,A<6m?†Ìdz!Cá?ïÔ+Ž#CÒ?gŽÇ&oSi?uê8ÛÐ3&?gŽÇ&oSiAGN4FGL J2050.4-2627?ïðn9ïdýÀBbBAÃï®À:)ÞÊü5À<=BùyÔ@"»ªŒÖ@skd?¼‡¾ºÌ€?ÆÅÓ^a_A@
d²ú"¯u@‹j:±VÐ?ïîÀ!ß'¿Ð'9@=‡Ë¿ãKÈUnÇ^¿á."2Q‹ä¿è|J°j¿ïÿúâôAGNfsrqPMN J2050-2628?ïòT
Ä):?[㘀Ö'?[WêÚ¢K?[㘀Ö'?ïé;Þ±v?r®›%	J¿?fÄ!BñÜ?r®›%	J¿?ïøœ Â?‰§RiÚ9G?ìKƒ²?‰§RiÚ9G?ïú€þ±æ?2By»ÏI•?G'üx«GJ?2By»ÏI•?ïб¿'a"?°Õ‡õÄö?w§ J>Û?°Õ‡õÄö?ïeÃ~D?–¢à*§½W?¦ÿDb?–¢à*§½W?î@Ÿ=®s?¢jUvcq?«ö"'sÔ?¢jUvcq?ïð*Ã3W?R=ˆÏ\?_÷ª,¢?R=ˆÏ\AGN4FGL J2052.2-5533¿ëËaè¨KÀCÇÞP'ÏÀ9M™æÆsÀ<-º9LQè@}»ÏN‡M@
hn~bÜ?§$H£v«ó?±ÒbŸÃý@$]È23Y@µ9"÷ƒ?ïÿ…]S˜¿ÛðŠ!«¢¿äÖ¹µ˜Ó¡¿äf;Óë¤ÿ¿æßyýò߆¿éà CAsAGNbcu3FGL J2051.8-5535PMN J2052-5533?ïþ¤•m‡d?"ÂÌãx?%¶§û0‡?"ÂÌãx?ïödë^µ?\8ÉIÞd?S6)V>fÊ?\8ÉIÞd?ïéٙӕ?gHá­pòJ?f&eõq>ƒ?gHá­pòJ?ïÿÌ#¸ž>ðþæ爸Ø>ùîö3Ȩ>ðþæ爸Ø?ïÿ.îÍJ?='øCœ?"&Ôö`?='øCœ?ïÞK䞿b?pàk‰…?pÚ
¢áß?pàk‰…?ïÐNÀ
$O?{²ºÊ8??wØ 
 ‡?{²ºÊ8??ïÿÂîQ¬Æ>ùµËó>þˆÈ>YŒ¼>ùµËóAGN4FGL J2052.5+0810?ÛÌX¿oþ&À6H†zØä2À;Ӆü-ãhÀ<ÔÔoX}p@#­w§Ši?ì6q¬?æ\-Þ	¶?ïèø5u@Ä	_$RÆ@Êmˆn£ø¿¤	àmW`¿ïr}šàl¿ïj¼Â´Ž?ï÷V¾}©¤?ƁWƒt"¿Ñd§I……AGNbllRX J2052.7+0810?ï錄ø#?{ËÍ­w8ó?fs{ÿ&$¦?{ËÍ­w8ó?ï¾pXI»?"?ã}ä?€cÛõDGP?"?ã}ä?ïI8øN?«^¸Ô¹?–ØüyñZ6?«^¸Ô¹?ï÷¨•àÒh?I'©÷¦Öº?P®Ô Ÿ¦?I'©÷¦Öº?ï¥^õ¿ñX?,\ä¹På?†¨BÂ×?,\ä¹På?îjʋÿÓ	?¶fQßøæ?©SW@Ïh?¶fQßøæ?ï"Ùàö?"ÃK'Ò4~?œ
Ã;?"ÃK'Ò4~?ïÕ]èÇî?y:Ó«Pà?uQ}
O?y:Ó«PàAGN4FGL J2053.8+2922¿Ý°› §LWÀ#´§qÉpøÀ9[¡ÔÑ~À;½Ca~ @ ïû_‡O?÷7קò!ñ?¹e1³rí?ËcËV€b@ÖKìgœÇ@	äQ»ßi²¿îâ/àm¿àÜ ý¦‰l?мj^ÄпÂåр´¿Ù1:_¢Qú¿Þ³+;-CAGNbll3FGL J2053.9+2922RX J2053.8+2923?ï‰Ì9©ïÓ?¦±ë§±Éâ?ŒñœcC3?¦±ë§±Éâ?ïDQh¨`?ª–ñ£º½}?œ—uÏ{X?ª–ñ£º½}?îÍÕòv'?¡Y&YRy?®""Ÿ È÷?¡Y&YRy?ïŒÃ9r‰Ø?v!Дp¦?ŒÏ1­¬^?v!Дp¦?í¥3hÁÎ?±^™»Iå?²Öd¿sþ?±^™»Iå?ëçþ‹$¥–?ƌßT—d"?À`Ómiª?ƌßT—d"?ìê¡¥ñZ?©!H´,ã?¸ªòÐu+"?©!H´,ã?íÃaŸéP!? Ü"Vº—ƒ?±äómLò? Ü"Vº—ƒAGN4FGL J2054.0+7024?ʂtËL$@0cجëÀ;½¾<RÀ<L™iÈñv@ 
<ÿdÐ@í-zŒŽ?ÅÀæå|Ç¿èhV"ú?ÊkÅJøL?󏐬5'ª?ïâp½Ø=C¿ì€"'‹á¿ÉÕ`ÅÂu¿é"²a'•i¿ßdIÁ1濧ÔŒ:
"AGNbcuNVSS J205350+702404?ïïH@»?¿FÚãn'?¢õø°¤?¿FÚãn'?ïÓe':‹¨?zŠkluJ5?vM7wWÓ»?zŠkluJ5?F/öN?‹X¾´»q?‰®fCü?‹X¾´»q?ïšè'Šø0?p§Ta8ý?‰Eö$!+ü?p§Ta8ý?ïí/BôØ?aøþ5§æ?bìÐø$oC?aøþ5§æ?î¹ZL°:x?¬'–Û©S?¤j[9GÛr?¬'–Û©S?ï‹h)Ï¿?v‰Ð÷õ]?%õÅÚä>?v‰Ð÷õ]?ìꛌ¸à‡?¥Ëµþ,ªÔ?¸«#š8ûÊ?¥Ëµþ,ªÔAGN4FGL J2054.5+4731?ëò¨¦Ò½'?úG-ÉÀ:|sÁ˜¼$À;àý÷Cõ@"
d|¬Mü?þÆ*\}?Ì1°|4.?¥&8à™?ØÏ1Ì*æ@¥4L?äæ†ý_¼©¿Äè'Ç¿ï³Ü:þÚ?äc=¬ˆà¿àւ""F¿äØ'sâAGNbcuNVSS J205432+473338?ïü[ôٗr?:H†¥¢Æ§?= X"–§?:H†¥¢Æ§?ïÞþD¶_Å?}'ƒ½¿"?p€Ý»}‰4?}'ƒ½¿"?ïÒÙÑÃÆ?{_wÀÉâ?v"0Èý?{_wÀÉâ?ïô~Ðs(?Dä j{?W_MéÒø?Dä j{?ïòjÓTóš?avDQ~ýÖ?[*Y^W܅?avDQ~ýÖ?îÕÍPo?²Dïɔ«?¢£*ø2H€?²Dïɔ«?ïtšB®H?u‹àWõß?'},·ª7?u‹àWõß?ïÏ;¬k?qHÌõn†?xâ+ª'?qHÌõn†AGN4FGL J2054.8+0015¿Ñü¿¤ÀÀ;äÚ	Ì2À:")¦ÂwÀ<O®‰ë¦­@!GáõRýÔ?ý!þ¨+¡?ÀY ãOp¿o+'\2¨@?²H`þàì@P¹Qð¸?嬗moo$¿ëåáℿÅf˜egÿ¿Þÿ²þ æ¿Ôâ5_wn¿Ú¢5_wnAGNbll3FGL J2055.0+0016RGB J2054+002?ïûN»'€+?7†í<͔­?BÅ‰i?7†í<͔­?ïèêHÍh?iÅ=Šš»?g·‰@?iÅ=Šš»?ïñô_@Šè?X­‹	˜¹?\A[.?Õ?X­‹	˜¹?ï÷Ý>+0?4óNª»B,?PEƒE5Æ>?4óNª»B,?ïñ‹U?S'ÌdªÌ?\éÏÃËg	?S'ÌdªÌ?ï‰ԇ½_?'`NKð? 
ëÏ?'`NKð?ï𚿴`o?kÛÊ«ß;??^ʀËy1?kÛÊ«ß;??ïëыèô?R¡zF¼&?d.tf«ü?R¡zF¼&AGN4FGL J2055.4-0020¿æX'´èLÀ;sP]¥À:F0l¯UÄÀ<<¥5¯@ ê&dä?ûäÀ>Ië?ču‰nÿ?´wÀÁP»?ôô¿%D]@Lyµùw¿ïܕ'2Ê®?ïú«bùÌ¿êRÆ«ú?±1¦@F¿àûã:Í[h¿Ù·ÿÛ<§AGNbll3FGL J2055.2-00191RXS J205528.2-002123?ïõâ…EϘ?¾¶3è—?T:õ•]Ì?¾¶3è—?ïáåu$ü?zBáq Ñ?nŠrš´D?zBáq Ñ?ï½3ã9ÿ3?ˆ¤M4¼œ?€³5Ÿ»D?ˆ¤M4¼œ?ïïIËP ?Gù¨Ô·£›?`øµÿøL?Gù¨Ô·£›?ïñ€»Å/?^š©Uû?\þ‰Áµñ'?^š©Uû?ïm­a?–Öþ:>P"?'OÊNµs)?–Öþ:>P"?ï‹?
:??'ü"»Ža?0?€!:?'ü"»Ža?ï¾x.B'(?t0OȲ?€aôt+*?t0OȲAGN4FGL J2055.4-0504?çjõ×)"pÀ=ÎðZpŽÞÀ:÷ÀªšëÀ<˜ëô°@•\­€k@ö¤¼ãJ¾?ÈWûØð?±*ð¬IJ?å¨D€b'?û/3÷Ô7z¿äûÎã''%¿Û•ýÈX¿çk(½Žkh¿ã'ßx ûŽ¿à?¾øMÚ¿å%:|CGAGNbllNVSS J205523-050618?ïû=¿djŸ?8?ÛÉ,÷'?C	ŒW\?8?ÛÉ,÷'?ï×ßÉîdç?u±z,](j?t
ÝP–?u±z,](j?ïÖßCX* ?t˜e?t^dhÐ?t˜e?ïåríÕ¨`?P¶ûó·m?jIô×?P¶ûó·m?ïòçsõ£¹?S>ó²"ó?Z1Úÿå?S>ó²"ó?ïà"{;F? ïzËÈ÷È?cû°˜—D? ïzËÈ÷È?ï¼Ñ[k¥Y?:±Åsî?€Ë©&‹¨?:±Åsî?ï)8'ŸÏ`?‰<4Õö¡?šØ猪x?‰<4Õö¡AGN4FGL J2055.8+1545?î˜?ñÿٌÀ2"f¥P‡À:‹Ÿ_¬8À<>À//˜t@E'Äë@¢e㉧´?ÌÕY8U†ð?˚KäÚá?ü=W(ÛÁ\@Rr{r'¿áëCII?Þîs恩¹¿çÆIƯc¿çv?!}ÿ	¿ïþadžæ
?ïô€ÜqAGNbcuTXS 2053+156?ïóE&ФH?Wkë‹OV?Yu±ëD'?Wkë‹OV?ïÙ\±B?z¬%å¦8=?sQ§tóüÍ?z¬%å¦8=?ï«Ê$5?xyÓ`?…<̈́»b­?xyÓ`?ïãÿ^ÍôH?T');üC'?l¡vÃçÝ?T');üC'?ïé­Àíñ`?fò%«Ú?fR?!,èB?fò%«Ú?î¹å˜ºe[?¬¬WYª¬—?¤a¦ví_N?¬¬WYª¬—?îÊ#‹üM?–Ú¡túëÓ?£]È
¯×*?–Ú¡túëÓ?ïTñ&¦æ?7¬gó{?žõaàR,?7¬gó{AGN4FGL J2056.2-4714?ç‡!‹@ÀD1&|k‹iÀ7Š8|HOûÀ;"K}¬Ô	@k?jyž@ÒΤ=aŠ?"'p€Eµ—?»|ûÔ!Tä@"Ô¦°)(@Â*/ÔY¿Ä>ŸøÙE+¿â›SíNM¿çX'AƒÍ¿ça''zï
¿é‹¤ô^¿ë4ÑΔM)AGNfsrq3FGL J2056.2-4714PKS 2052-47?ïôEFR—?duIa˜-?WusMSü?duIa˜-?ïá@)ïEP?€˜gÕN>
?n¿Õý|ßÑ?€˜gÕN>
?ï¤&®Ú7?ŠÈUCÔ@4?†ýöW¹$?ŠÈUCÔ@4?ïú·VC´?<ÔckY?E"¦¾é§?<ÔckY?ïð˜ó›1Ž?X
1ùùˆô?^ÎýÖó«?X
1ùùˆô?ïb™jt½í?±+
T¶ž_?"¬Ò­ø¦c?±+
T¶ž_?ïÇR…;œA?ƒhó·ÜË?|V½J$›©?ƒhó·ÜË?ïÖ2%/ÿ?lÐ`	:öP?tæ퇜ßÒ?lÐ`	:öPAGN4FGL J2056.4-4904¿·l¸Ÿu$ÀD)GA1MÀ:Õ¶;ÏÆÀ<IjÃQ#@Q/@4xƒ@QÈ"n·?Ù1ŸY?î+hߝâ?ÿoœp
¯@ñËß¼é¿êå¡z8«B¿Åö
³¸(Ñ¿é­VN¿í3oce*&¿ï齞[ :¿îíÑ9*AGNbcu3FGL J2054.8-4908SUMSS J205613-490415?ïò®¿æ?`Š´rç"Ö?Z£ô±®;z?`Š´rç"Ö?ïÛNB¶¼s?}u5Š)¸?rXÞµæ‰?}u5Š)¸?îmcNj,€?˜hLëÙ?©)Ë?˜hLëÙ?ïnÑÜxˆÊ?€mvFt€Ë?'%Ät^'´?€mvFt€Ë?ïuê'{™ÿ?œ#WùF?'B»eV?œ#WùF?ï\Hèý"?¡çxÇJx?"vâ×ÈuÇ?¡çxÇJx?í:*‹nޅ?¡ûiú6ì?¶.«£?1Z?¡ûiú6ì?ìZ¾Ö¯W?¯‡,nBßÁ?½*YJ…F?¯‡,nBßÁAGN4FGL J2056.5-0202¿è™QgÑ qÀ<Ž¹¡vÝ­À9ç
›dtõÀ<:"ŒòÂ*@M@NN†@‰êdHR?»äC`ýÆÀ?À¼Ÿ9@>@ ¾×@Ä@I'zìZ\¿k
Ñ¥'¿ß*m¼Æð?¿çÒ·'¨ä¿è0¾yLòø¿çôÝøn;G¿ðAGNbcuPMN J2056-0205?ïý—Ò¼rY?*®è|I?3AjÏ¥£ª?*®è|I?ïåÖZY¼?t»ü¸%_†?j)¥}Ãô8?t»ü¸%_†?ïå°Ü+dˆ?]´hþÍJ(?jO$Tçñ?]´hþÍJ(?ï÷™€*mù?6ôÃÂNz?PÌÿÎßýþ?6ôÃÂNz?ïøùfñ¼?J‡¶jÒ05?LfÔ}è?J‡¶jÒ05?jiïø?"º'`@?%e"?"º'`@?ïfv«qÍ?ÃÑ8‡Ôø?"1*–íÇã?ÃÑ8‡Ôø?ïÛæãäT?_ëÃÁ	ù?rŽ"Š­?_ëÃÁ	ùAGN4FGL J2056.7-3209?î[68'ÒÀC¯!JÓcÀ:ŸZ·ÜzÀÀ<G{4SÄ£@ô¨^•@¤Ø&"»?ÅûœÙj?³Úx±íxi?äú›qàíì?ý¨å|qÀ¿àh)µ/ë¿çóÂâæ¿äŠ‰Ü¿ïÿÿÊPË?ïÿçÁŲ§?ÀÍ<HۑAGNbllPKS 2053-323?ïýi%™¨Ä?Aâù'‹
?4¶Ò)Ls?Aâù'‹
?ïèVÛÙÚý?wŒ"³jr?g©$ˆšð?wŒ"³jr?îƒRr
*ô?¡"+Â*ÑH?§ÊØÝ¥'É?¡"+Â*ÑH?ïÿ‡O:J?
ê€Ç¤Ýô?,,{'a?
ê€Ç¤Ýô?ï÷Ï|KøH?UcñÒQ±?PaÍ}€'?UcñÒQ±?ïLBCˆ?£Pþ 1Ü?–w·š×o?£Pþ 1Ü?îÛ²|OÂò?™»|ÒÀU?¢DØ6¸Må?™»|ÒÀU?ïõ=I6ª·?\˜ôCUY?U…m:´'‰?\˜ôCUYAGN4FGL J2056.7+4939?ʹ7¢6SØ@	<"?¾À8c}}Ú À;i!Æ#e`@!p±E\Öp?ýMoõ[aP?¨³"?ãDÞ?¡=¢^6?ö­§%sW@	¦"Ö/?Þq&þòcà?ïð¦%™½¿Ëä¯A¡‹¿Û'$l ¿à]*"As¿Ô¾Ô;«ýŸAGNbcu3FGL J2056.7+4938RGB J2056+496?ïýüug?(kt֓R?0VM‡Q?(kt֓R?ïØ-g[?{u¾›£3r?sóiS1©'?{u¾›£3r?ï\T›R?",¢ê3±?"~5l•Í?",¢ê3±?ï}»ìn—|?'Ÿ´ÓiCš?H'm¦ƒ?'Ÿ´ÓiCš?ï÷ö^k›/?J•ê''2Ù?PC¥Nì?J•ê''2Ù?î‹õÒ³Y?³ÄPäÍ^=?§@¢Ð'—}?³ÄPäÍ^=?ï<"Ê
;
?š-oõ'[?˜mf¹14a?š-oõ'[?îþr8y®?˜‡ª9í!? Üw"%?˜‡ª9í!AGN4FGL J2057.4-0723¿î¶¬0Ü'À?P]…TÖÀ:'%üéË
À<Eí@
@o"&¾Þ@pHðŽ?›™#'"?ÁÉÁÕwì ?ùLÝF—"@SãÉ®¿ÏºÆdþ²M¿åëðž¹2¿é(ôëÏÇS¿êîb›Ö‹¿ïë[rž¿îߋ€Ò"wAGNbcuPMN J2057-0719?ïü ÿ‡?:øæˆc?;ÊÇO«?:øæˆc?ïâ'‡×z?m]¸bG æ?mãmb+Ï?m]¸bG æ?ïÖæÜ(Ç?r›†dsø?tðŒ°(,"?r›†dsø?ïÚ,¢±~?\ãáxï©?ré® `		?\ãáxï©?ïðØPKz?fƒu™ ×§?^O`QÚ¬I?fƒu™ ×§?ïr?êóöª?"ÕV'ƒ_?'¸¦¨"Â?"ÕV'ƒ_?ï¤ÜuX¿?‡êûÂö¸˜?†Èâ­?Ûç?‡êûÂö¸˜?ï¨tQ?‹Æ[º(÷?Ÿjñnuð?‹Æ[º(÷AGN4FGL J2058.8-1442¿Ú
mó‰¶3ÀA`Ľ3ҕÀ;#jęødÀ<˜dH~ôÓ@ ¬ˆ0½7@u×ÙôÓ?ÄrvŽ*¦¿«;Ž÷T4á?æ!EÊål?ÿ'g΀¿ÛÔñhˆ¿äpÝî]@M¿Û%⽤檿ۜ–ƒå}H¿â~äw
}—¿ÖH'¶þ.oAGNbcuTXS 2056-149?ïúlí??>6Áí|˜ø?FLLI?Q?>6Áí|˜ø?ïçâÔdàn?iƒnŠ¦Os?h+½{©¢?iƒnŠ¦Os?ïé'4i>?cââGJè?fmÌ("?cââGJè?ïîAl
‹?G4+z4Æ?a¾"з%?G4+z4Æ?ï÷ûÁ
Í?Føó®"f¬?Pü¸0"
?Føó®"f¬?ï|Y¡uÊÌ?"Ñ$Ò!€?tËØ%Þp?"Ñ$Ò!€?ïëH{¢kX?n¼µÝWîƒ?d·"tñÿï?n¼µÝWîƒ?Ž3Æ?zرVÒ?‹Tv~¥?zرVÒAGN4FGL J2100.0+2103?¥ÉÇû$û—À0#æÿëÀ:‹DÙMäÀ<(6'cDs@1Þ ôp@Ž ¤»5Ì?ί¹<:ï?ÀâÔánD?õø¶DË,@Íé/.è?íÿí@_Á‡¿ë>"E]¿Ù ²ýî­È¿ë€ y\¸¿Ý»lb&¿ðAGNbcuMG3 J210007+2058?ïñ–
W?™©Ô ê`z?\ÓÅÇnú?™©Ô ê`z?ïä³hV?u¼ƒæîMÞ?kîM
TÙª?u¼ƒæîMÞ?ïّû¯R,?yË´óG?s70•ùÄ?yË´óG?ïö X:(Æ?9jB%­ÑA?S¿OØ¥´?9jB%­ÑA?ïüšlu?BâàV²3??Û0FZf`?BâàV²3?ïmóŸ/ÁË?¢ÉÁöøñ?'AŒOø©?¢ÉÁöøñ?ï©Ä +`?‡b—€¸íµ?…ŽØ
ó—õ?‡b—€¸íµ?ïÒ ŒäÆ?eV—MNfd?v¯¹"Y57?eV—MNfdAGN4FGL J2101.3+0912?ÚZʨý‡!À7ƒï(Ag©À:ã´+W€À<v*¦€2@ 25\XF@ÍÝ|è‰?ÁI¡¿¨ä;ÃS?åž6Kìg?ý¿SrB舿èÊ(­ž3\¿éãîâvWJ¿Þܳàֆ¿Ûú\}‹Ñ¿á¤TÞ~¥ø¿æÆÂâh?"AGNbcuRX J2101.3+0913?ïûÀ2_£ª?9Y'!§¶u?@ÿ5}h"·?9Y'!§¶u?ïÜpt9ì>?t¯ÆוR¸?qÇÅðÈQ(?t¯ÆוR¸?ïæå8˜;º?sêsϤ#?iÇ ÝX?sêsϤ#?ï챦¼Ô?Is'"½4?cûN'ÈÌX?Is'"½4?ïíÌ"û$?`ÎÑÝ¡g	?b3ÜСÕÀ?`ÎÑÝ¡g	?ï5Š®ø¯?œó•5F§?™Nª ê2?œó•5F§?ï凩à—8?u'"7ò@?jxVN#x"?u'"7ò@?ïw'ØÏz?Žå?'
Åý¹?ŽåAGN4FGL J2101.4-2935¿ïî¸Ù0ÀCï–AöD•À:pÜÀ<4!'÷¾é@ìò²°@Ƙã'4p?ÂNÙ¬Ú?ÇRÇ%Ãß@.Lÿy@
朌h-¼?ëR¼ÐÖFÉ¿ç.÷™ÿðç¿êí3¿Ë¤¿ç¿jäz¿ïÿþˆ0»Š?ïÿ¥ÂqÕAGNfsrqPKS 2058-297?ïß4«$ÓÁ?q(=
`?peªtuWL?q(=
`?ïèNŒÄ¸Æ?n#‹_3?g±swÀY¹?n#‹_3?<íÇ?'Ñcöµ?‹pÇýÕå?'Ñcöµ?ïïß®HI½?JSSSx<?` Qز'¢?JSSSx<?ïЈF"Ò?€ B)Ã
h?w»¹JØ?€ B)Ã
h?ïc,Mn{f?˜÷Mç¯ö)?"švYË+?˜÷Mç¯ö)?îÁ9Gì ?š'ª
ºe³?£çìm9ü?š'ª
ºe³?ïs?EmÐñ?'´ÿ4€Ë¤?'˜Y%Ç?'´ÿ4€Ë¤AGN4FGL J2102.3+4702?ïþå}³+?՝ò#žjºÀ8¸lD̹À;9•zP(6@Fx M'{@'ï[m ?´1[}æF?®ú	pìý?÷òZ
7'g@¼¾"ºêø¿Út_Cý?ïþdž;îÄ¿áõ
=€>)¿ãmŽä3ñŸ¿ã´ =¸g¿åálˆ€ÃAGNbcu2FGL J2103.4+4706MG4 J210218+4702?ïñ?û:ñ?hŸÙPËó?]€	ª­–?hŸÙPËó?ï»Ó€E4½?"ᜏ-µ?æ˶­?"ᜏ-µ?î»JovÂ?Ÿ8¾¼	?¤KY2XÛ?Ÿ8¾¼	?ï'4W¡†?…GËp‰?›uTC?…GËp‰?A¥Ý?Š.húé‹b?ŠÝo°‡´Ï?Š.húé‹b?î2ÒKx	¸?³£fý./?¬ÒÛG£}?³£fý./?íþ$¹{iá?¦b˜l*n?°Ú5—ô?¦b˜l*n?ìp@ƒ#?ªüÊåm¸?¼õûçŽç?ªüÊåm¸AGN4FGL J2103.0+0342¿ìZñ"ǺÀ:îÊFà!À:j;4¦À<=EŒÒ
ú@e`ïYÂ@¡¬Wâ?%?ƒo‹©?­Ï‡Ò?å—?¢,e@౫´#^¿ÜqÃL¿ä¢C çU¿æþ½c£>¿ãÛT"¼'ÿïnoês¦Á?é|ðKWgAGNbcuNVSS J210301+034411?ïû¶Ü9k?9v×+¹È?A$,Ç?9v×+¹È?ïã²
9ûà?}†š%= Ò?lMö	\w1?}†š%= Ò?ïäV'ÝYQ?neX|°å?k©}5ä"?neX|°å?ïø±ç"Û?9m¢Ðuš'?M8a/ÖP!?9m¢Ðuš'?ï÷ZÑ¡Œœ?V¥§®Ø¥?QJ\¯(X+?V¥§®Ø¥?ïsQّG?–)±¥
-Y?'•ÄÒ÷A?–)±¥
-Y?ïáÃO±ªC?tÙë+À?n<°<wÅS?tÙë+À?ïÎÎPŸC–?iÝ®\ÏWÏ?x˜×·íX½?iÝ®\ÏWÏAGN4FGL J2103.2-2114?ÚrY¬Í0¨ÀC•_x5œÀ:ûXª¼ÍÀ<Ó׃	4@sS¶
"'@U>S!æ?È¿4ïb¤?£›¼£M¼:?Ûj•4°
õ?ý¢ë$PÂ:?ï?Äpݸ­¿æ\IÂkÊÔ¿â%!!¸·¿Ú¤±ÛYØd¿áœ?':z¿ïú"á%Ê?AGNbcuNVSS J210312-211216?ïöñî·û?N†às *Ó?Rãʚ	'?N†às *Ó?ï㮀†x*?uØü®ƒ_í?lQy‡ÖN?uØü®ƒ_í?ïՁÀp.L?u?åP'Ë‹?u?Õ§I­?u?åP'Ë‹?ïÜ>S
?UË~|àa?qàðNëÎ*?UË~|àa?ïíCíÀN?_è'pÀ?b¼9áû?_è'pÀ?ïjm›}¹-?˜<+ŽÕï?'²L‡±Ôh?˜<+ŽÕï?ﺏ?"BO?yøcd??"BO?ï_s¬[Nl?€‹Ÿ#Oõ?"Šm¶ú™?€‹Ÿ#OõAGN4FGL J2103.4-7816?ì™O"4LÀ@'óÜNôÀ;ºòù‡?ûÀ=Wg:¡¼~@M°À§¥v@,—½÷Fô?Øü>ª_º{?ïÿÁ¶ïö@—»=XP#?þΚ,f?ïغadw¿äz7i"ÙI?à)Ñ =ô¿çÍ˚¥˜¿ïÿßéà
¿ïÉöž'ašAGNbcuPKS 2059-78?í_:žÈ"¾?¿îy2Ø?µ+
)U?¿îy2Ø?êñ	±ÉU
?ÄòØq"¯?Ä;Ù8Ú«Ì?ÄòØq"¯?ìvUÐI¸?¥T䖔—×?¿MQ}²D?¥T䖔—×?à1õN(à?½#5½¦Œ?ÞŜc®??½#5½¦Œ?èvG=ýˆ?Ê{Ú½Œy1?Î&ãÜ	ß?Ê{Ú½Œy1?á
{—É?ÒlÞùJ.?Üßå	üÐm?ÒlÞùJ.?çK¤ß{ƒ¸?·ÌáœQ?Ñh¶Aø'?·ÌáœQ?Ç{•WQ?º3CŠ†"?ê!;Úª8¬?º3CŠ†"MIXED4FGL J2103.7-1112?ï"µjc)ÀA4Z¬1À9ßñQçSaÀ<hdÓ¿/U@ÍB§šcC?üŽ`¶#=?¼¸KTg?ÝóB¢'åÆ@ @9«ó8@r¤íà˜²¿ç7àìêO¿¡qëCŸ*í¿ËJl_Ϟc¿æs?ã­¿ë¯eŽ$Æ¿ïÿœ}y¨cAGNbcu3FGL J2103.7-11131RXS J210346.8-111335?švƒc#I?¯LŠ§vAŸ?ï,Käô¥ž?¯LŠ§vAŸ?Ѝ–‹È¿?Æe'iW:,?ç¹4ºð!?Æe'iW:,?ƾ5~Ö¹y?¯¯Ö²?êPr JQ¢?¯¯Ö²?ÞÝx?·däd¦Å=?àö'zCñz?·däd¦Å=?fuòµ¡ ?dý¹).?ïéŠ
=2ï?dý¹).?¤±î•˜"Ñ?§uVÂz%š?î´áÁô"?§uVÂz%š? sU»‡ûÃ?"ÏšàÖÿ?îøʤ~z?"ÏšàÖÿ?­z}‡…¾ó?ÀÐobœ)?î(X'£ ñ?ÀÐobœ)PSR4FGL J2103.8-6233?îy–ŸÇ¹›ÀCyÅoÀ8ó¤>aeÀ;éµ³¬@wèºéö?ýº›
7 ?¦¢,+ܨ?»¢é#šŽâ@¯.Ìț@
{H!+ô¦¿Ù/F>¨²;?ðFyŒ¿ß¹õ¤ÝD"¿ßêoŸõÿ ¿åU¦$ÂW(¿àò''sã'AGNbll3FGL J2103.9-6233PMN J2103-6232?ïò¥¥ªŽ?x€§‹ÆÜl?Zµð¦ìtz?x€§‹ÆÜl?ïØT´àó?~' k?sÕÿ$/®?~' k?ïEñ\µHÞ?•×ê{Í?—AÔbw¬O?•×ê{Í?ïÓWÓ\?_–çwBã?vTvô±ù?_–çwBã?ïÙ ›è®?q¾=Ì?s?so²*å$ë?q¾=Ì?s?ï<dÇÍ?¬ÇpQ?˜s}¤f>]?¬ÇpQ?ïg.â]?'œэPá?"Z4ëe?'œэPá?îÊÕèÄ?'²'ùl\?£R¡q+É?'²'ùl\AGN4FGL J2104.0-3546¿Y<$‰zOÀD´%®æ1ùÀ9Ì "ˆÞ`À<FŸ°4@™ãtÙñ£@ÁDÙMä?³·»B¶³Ü?¡5žPJ?êÈÇ.¥/@ùçb$b¿ÑB°Ž¨¥¿áÊa¸¼¿æċ_Å¿àú,hJl¿èÅ-0º²ï¿ïÿÓ?,» AGNbcu3FGL J2103.9-3546NVSS J210353-354620?ïúKzý¢-?]›s´¿x?FÒz1?]›s´¿x?ïê×>sa?tè©ÊXÇ?eà(퇞ð?tè©ÊXÇ?ïÑÿ‹)Ù?wÊXH¬oG?w:‰P¾?wÊXH¬oG?ïþ¨$ªb?u'Øàâo?&%}û¸Fî?u'Øàâo?ïùf9V+?RHZ#òTo?Jg/!Ñ¢?RHZ#òTo?ïg·•Ì?¢_³ÍU†?"	©ìʄ?¢_³ÍU†?ïÁd˜tÅ>?D"öŸ£?M³«€YQ?D"öŸ£?ïý>ۙ)˜?,¨ñÙ=%?6	"ÅsP¡?,¨ñÙ=%AGN4FGL J2104.3-0212¿îý[Wêw®À>Q2ƒ
À:«§…§WÀ<` ä¶1@!ë_ð«y?ù1†U7	?ÃÉS¯-Õ?¶Îu'ãö?ó£Þ–ù¬@Ògd¾­?ïÒÀÓoS¿î,QA¼
¿›j˜ò|¿¹Ëx1¯·¿Õz«Â»üÆ¿Û쑎2]AGNbll3FGL J2104.2-0211NVSS J210421-021239?ïüÔrÄ©Ï?/óñ׸ˆÜ?9\h.ûÅ2?/óñ׸ˆÜ?ïåït†T?l±ën¥°?jé…úL'?l±ën¥°?ïíûeçe?cÚ1é?bšD•€b?cÚ1é?ïî0U™uÄ?F°ó6¯?aϪu¨"^?F°ó6¯?ïùNû22O?Bg¬˜ï	—?JÄó:ýð?Bg¬˜ï	—?ïڜ æ?äƒñzk?¬z+q?äƒñzk?ïæÐYTT?uËKÃüÝI?i/¦Ö¬ì%?uËKÃüÝI?ïÒÎi%?gR€9Nå?vöеJ?gR€9NåAGN4FGL J2104.7+0108?ìªäU條À<ªà¹ÜÀ;®ìÀ<~̕ohn@Kîí3»?þ…ä*·c¯?ԉ݁%?Ìãݵ}Oâ?÷£›0r@µ
$F0f¿ï ŒÒá¹Ä?îsóãqT?Õ%çۛò¿àè`Ļܿç[gà$¿àQþÐUAGNbcuPKS B2102+009?ïþ<ÍÕz4?)v7 M@?,3'ì?)v7 M@?ïä|z`)?päPù?kƒ…ÖÐ#?päPù?ïÝéH¸?fH;/7oh?qyÈ{Sè?fH;/7oh?ï캠FÔG?Jq×>—†Q?cE_'PA?Jq×>—†Q?ïýŸLa?0S¸Ëš?3?ê)ON?0S¸Ëš?ï"T»™É?'fÿÍÜë?ŽêÑ —ÅÇ?'fÿÍÜë?ï¶Åñ³®e?ªj±«‡x?'Nƒ'¢º?ªj±«‡x?ïÐ1—+?i(Š}éÛ?wçp»I¯±?i(Š}éÛAGN4FGL J2105.2-5143?â÷«ŸDm1ÀD¹Â.äÀ;.á"ÚîÀ<‰"'Þº@yÝîÞ¦@E¦'¶(F?ŤK¹¼Ïª?më«¿säL?ª%vkí@ô¶ùPäI¿à|¿n?x¼¿èr@úœñ¿å­A—$¿ç™¯Ôn¾¿ÚQ¯<Ü)¿âÚÒê?¬AGNbcuPMN J2105-5145?ïþ)ÎÛoÓ?*óݕ«È?-c)O¸s?*óݕ«È?ïõê¯O¨#?X‰,F¦?T*¡P1š§?X‰,F¦?ïìÁñôÆÞ?gÙåõä?c>)u±"?gÙåõä?ïÿPªèKƒ?»*¢<Sà?êætà?»*¢<Sà?ïþ¼œåÉ?$wo0ÐG?$64¡WB·?$wo0ÐG?ïÚ[v•«?tøW@‹çÑ?rþRe±j[?tøW@‹çÑ?ïéCÈN/Z?qíiYÎ?f¼7¬QE°?qíiYÎ?ïûnZs
†?9uì×wÅ«?BF–Ý)
F?9uì×wÅ«AGN4FGL J2107.6-4148¿µZ Ù€™«ÀE>$_ZÙjÀ:'
[2U¾À<|2;¼n±@N ?ûîx@Êi`êM?Å–)̓×?»¸€ºz¾?ópnAüú'?þ0«#uü¿ÏkõÇl房à/ž˜\¿äo¾Sã,¿å`ºÀZ΃¿ê²M?Mó©¿ïÿ&ñÜPÎAGNbcuPMN J2107-4145?ïú-˜"‹é?Dõ~Ɨµt?GIø"©µ?Dõ~Ɨµt?ïÝ©ü»?€}D¢'ýÓ?q+}áEx?€}D¢'ýÓ?ï¦ë•v¥?€‰¦î%ø?†E˜0¿?€‰¦î%ø?ïٞ"Pž?W@¤'Â
?s0îó-Ø­?W@¤'Â
?ïöp™4Þ?[Ò̆¤öú?SÍB¹ô
?[Ò̆¤öú?ïø«øÁÈ?šf	:Uë?ŒÔ÷€º?šf	:Uë?ïGûQo‰P?'6xœzÈ¿?—•Ú¥Ûû?'6xœzÈ¿?îú§³Z,i?êroÌ%? U"Ìr?êroÌ%AGN4FGL J2107.9+6006¿ä(Yã÷@ ØÀßXÀ‹À9î²-å™À;'KZqež@"eæ
æ@ß8úóPÅ?Ë$kYÀ:Ã?ÒS:»@gæ³þŸ®?ú˜€â¾{¦?çôS>kuš¿ÑDŒÂÂ#¿é´÷!¿æ_iQÓ1k¿ï÷äÞ;Š¿ìue<š»AGNbcu4C +59.33?îüH­î»4?§¢°~"? ;u"̼?§¢°~"?áXü^Æðü?ÌÉÙ#-'Æ?ÝNBr?ÌÉÙ#-'Æ?íQٔ¹éy?ŸüÀ€DP??µq3YTÍ:?ŸüÀ€DP??âOá®þ}?¬Â{—Ô\3?Û`<¢Õ?¬Â{—Ô\3?ëQ¥=€'á?ÃÔo6"?¹k	ýô|?ÃÔo6"?»ùèJ?Åivj"G?ì€Âö½¿œ?Åivj"G?Þ22ÝwêÈ?»ê"!ÏLs?àææ'D
œ?»ê"!ÏLs?ªx¾Ò•?[ó"Æ=?îXtÿê?[ó"Æ=MIXED4FGL J2108.0+3655?ê጖'/ÀÍ
Œ°}À:ÊÓÎHÎÀ<&¿»lR9@ x¿úeñ?üe&*64o?Á?öût€?ÃΕ¤Âl¢@ª‹ÄÄÀ@̝–~\&?éåïé1‡b¿æóóiâr¿Úª|€Y+À¿Û
ü]^*¿×Ù#"™Þ¿ëS9bøÝAGNbll3FGL J2108.0+3654TXS 2106+367?ï÷C'jÀ?PÜ՜ì±?QxÛ'}Ò?PÜ՜ì±?ïʪبš‹?ƒ§dUg?zª"ÉïJm?ƒ§dUg?ïâÑî
¨ú?qA‹oó"?m.ûõî%?qA‹oó"?ï°XìfP?b.½'{!ô?ƒéÄä§Þ!?b.½'{!ô?ïÈó~½JN?xKdQcú?{†@¦*M?xKdQcú?îù--=Y?­î@œÊë? g-.ãøu?­î@œÊë?ï&û5¯©?—äiƒ†`?› ™F›A{?—äiƒ†`?î«
˜Öv?Î®¾ÑÊ?¥O&tW?Î®¾ÑÊAGN4FGL J2108.2-2454¿ïdÊÝªÀD¼j~ùÛÀ9î/²u2²À<Sîe£ÈÈ@³P–‰@_êÄ.˜š?¸œ£å"5?§¯ýˆ¬a?ê¨Ñz±w@q¢Æi}¿Ù#ñÁùµ
¿ãô~ø-£§¿å¯Z@hOö¿ép'D¿é0aœ¨¿ïÿì^ãe@AGNbcuAT20G J210812-245233?ïü׶­&?2Õlzôà4?9BI[‡z¼?2Õlzôà4?ïì°9ež¸?gÇÛ®_vû?cOÆU©¬?gÇÛ®_vû?ïÜFGÀ'‰?oƒàݖlÀ?qÜÜ
)WÁ?oƒàݖlÀ?ïú;IÏyG?5«°·á4æ?GØÁŽ'³?5«°·á4æ?ïùÐöýø¿?DW­`´Ÿ.?H¼%ñ¦²?DW­`´Ÿ.?ï¡D2V`×?Ž²Ð³rnï?‡®ójgÊ6?Ž²Ð³rnï?ïÉà80ëR?}k¦Å¾5?{ãûx?}k¦Å¾5?ïì•Àyµ×?U"ºDÍúö?cj?'¨ÀÔ?U"ºDÍúöAGN4FGL J2108.3-4824?ánÉ_ŸÀE)Ëeè'À:ÈV%¦'¶À<P–ÔÃ;T@æÅÎ*ñ@B÷<@?ÉÔMI´ÔÞ?'4ëïý©?ÃÏÖ¢"@QRÔäv¿®pXœhß¿åF/ßÁœ¿è58@¹-´¿êÎô$)ªô¿æ§­ŽC$B¿ï]6=©¯AGNbcu3FGL J2107.7-4822PMN J2107-4827?ïñÀ&¹'?˜úê¸Ra?\³bš3Z?˜úê¸Ra?ïó8—~¿×?a­j£a?r?YŽÑÿ±±?a­j£a?r?ï¿#‹UG?€­"aå?€7A'1?€­"aå?ïüRÌßç?'m³@«?=išèžÎ5?'m³@«?ïþú²kÖ?$ìæ sš? T×Q£§?$ìæ sš?ïÔIÚ®Q?y2TÜëCÖ?uý[2õ+?y2TÜëCÖ?ï¹
Tý2p?ƒV—0ɤŒ?¼ª»‹ù÷?ƒV—0ɤŒ?ïà¶Ýˆm?a²)S"¡G?oI"5šxµ?a²)S"¡GAGN4FGL J2108.5+1434?è¶áèV¯ÔÀ5¾p'IÀ9¿%ª´tÀ<#M"M@tN?þó'@"9¦û`?»ÿüOq ?Æ #÷V
@@ç6žË@žâ¾ü?°‰c–}Zt¿ç‡ª^7éɵ ÝD¿èûDå^³¿ïþgä맃¿ïna'·'AGNfsrqOX 110?ï÷`Ê£°Q?K¶J-@Å?Q>j<ímÃ?K¶J-@Å?ïàá'趞?s4üк[ö?om\'-?s4üк[ö?ïÎ0s š;?pÌju?xçƇ:˜?pÌju?ïå@-ŽûÓ?SIÆ—½4?j¿ÒvƒŒ¶?SIÆ—½4?ïî*½:U?c›üÕèý?aÕCƒïÄ?c›üÕèý?ï'*É­2©?¤N˜Gí¦ø?›¦Ìxê?¤N˜Gí¦ø?ï?GP?'C¨Šóðo?œØ¶Ä¤?'C¨Šóðo?ïX^M4³ˆ?ìfõ\l?"ô6Uùòû?ìfõ\lAGN4FGL J2108.7-0250¿îì@Q÷À?–E"}À:Id?D¹mÀ<cÿå(
e@<*žµ@z͹[ÖÀ?·˜SH|p"¿•4beÙVQ?ÞùI,™»þ@ƒàṗ?îñ/'¤ŠŽ¿ß'r¡L%¿á´M¯¶;'¿á§UCÿ3Q¿ã61µ"±«¿Û×[µ2AGNbll3FGL J2108.6-0250TXS 2106-030?ï÷0T Z?E™iŽ¦?QŸV±bF?E™iŽ¦?ïæ(@Äsë?jao§?i׿"Îä»?jao§?ïçj$‹ûv?iJ¯ùoԌ?h•ÛQ¨q×?iJ¯ùoԌ?ïÛл™É•?WMüÎÏ[Ê?r¢,ëén?WMüÎÏ[Ê?ïâÆ_[–e?d–Ÿ,k?m9 p/‹\?d–Ÿ,k?ï‰R:E²M?'íãÍä1À?«qdD˜Î?'íãÍä1À?ï×{Ǝ³ü?yèBÝ~ƒ?tB¦ÿ?yèBÝ~ƒ?à³ß?ut9úá'?Žýcl*?ut9úá'AGN4FGL J2108.9-6638?æUÙXvcµÀCÄÑ¢À9‹á¸À<YŒ~þä@‡Ëz½5€@ãÔk&¿‡?«£cUdá?yž	>7á'?Ωu¯¯†@38üö¶*?éÅëÒK'Ï¿áS
æû¿äÚ?çvœ?¿Ü!¾@ÂèÈ¿âÂâ2ŸE¿äÎ%\°ÚÿAGNbll3FGL J2109.1-6638PKS 2104-668?ïú}#ŽœÞ?9âaÕw15?Fq¿€lC?9âaÕw15?ïõ¼vúo?X!2¥
Õ?Uކ±Ö'?X!2¥
Õ?ïÕÜÓL¡?yr^gw‡?uþx?yr^gw‡?ïîo_föb?QÏ«1óY?a síÖd?QÏ«1óY?ïñѧäY?RÅî`ï!Â?\\°'Ý3?RÅî`ï!Â?ïÔ_–ú"?"'<$'2?uÐ4'µô»?"'<$'2?ïÏYtîòð?~P¨hj?xSE€÷d?~P¨hj?ïÒÙv~a…?jP*Šü'?v"DØ܁t?jP*Šü'AGN4FGL J2109.6+0440¿À:¡^ˆ³À;䃧 À:f̧ãß8À<-Q{×@ЕYC@ÖÎãþAº?³ˆX(¶?žÚ܍"?ßÌ¿`Ón?ÿ`™56Ä?îÂL ˜?àöÚhµÌ¿æR,¾}¿à+›>µGu¿à¢–˜]Yw¿ïüàÎï½AGNbll3FGL J2110.0+0442GALEXASC J210940.09+044000.8?ïð…½Þa9?^Ðõ×Ëc?^ôƒÚÉo_?^Ðõ×Ëc?ïÕ»­?ydíRnÛØ?u|"[%?ydíRnÛØ?ïÍKæfž?xÅï¹ççã?yZç9?xÅï¹ççã?ï­ÊØÎ/E?iy^ªÌ(?"IÏãÊÄ?iy^ªÌ(?ï·¯kG?~˜$cáu¬?';k¦ð,?~˜$cáu¬?ï9ÿøk? dAÕÚ´ä?<øÁ¸À¨? dAÕÚ´ä?ïE{‹³†?•êÔ<Sw?—PŸgªWY?•êÔ<Sw?îŒÃÁÐZ?'¤²
Ñ×?§3ÃâÿzZ?'¤²
Ñ×AGN4FGL J2109.8-8618?»i¡óôó¡À=.î¢
À:ˆ^iAâùÀ<pär@!™lä.é"?ûdÏÝùDû?À÷g€æ¡?¥þ®Ç(H?æÿ'ö֌?ýltóG
?ílŸWŸ¿á}Ó %¤Õ¿á•,b³®¿Øp¤ý[¿È	û÷ݝ¿ß IaûcAGNbcu3FGL J2108.6-86192MASS J21101113-8618473?ïüþ…xò§?)Y‰6…?8ӍÆ	?)Y‰6…?ïñ€»Å/?^…ú¸½Ö?\þ‰i¿ñü?^…ú¸½Ö?ï•ž?j¤õ³þ¶?`z^(öâ?j¤õ³þ¶?ïò$ê½p?CûRð/N?[¶*®VÕ?CûRð/N?ïùS^T|¸?JU–8©Ó?J²…§Dœ¶?JU–8©Ó?ïÖ³ï{?t¦Ž÷ç?tò¦G÷>Q?t¦Ž÷ç?ïò(;Õ¼?nB1&ãI‰?Zůài?nB1&ãI‰?ïÉXì?k––œôsÙ?{xS{]ñ?k––œôsÙAGN4FGL J2110.2-1021c¿Ø¶¨s&=ÀA½¾ôœõoÀ:¢v0íÀ<@õ0™%@t››&Œ‡@°HàC¢?Ëç"Ï/~?Å.¾¯R¾?ð…£dôv@ZKë»ÐP?ë™H`–Üx¦ojñæ¿æÌ<6çô¿ìŸÂÞ6œ¿ïôÁ]'çü?ïÐù^#øAGNfsrq3FGL J2110.3-1013PKS 2107-105?ïêðÝ,?i'VÛT2?eîû[Ð?i'VÛT2?ïá+nmÆØ?q‡š%¡?nԑu\p=?q‡š%¡?ïlã¼1÷?†m>?'cˆ}¡ó.?†m>?ïÒ¢M-–w?`óÜ÷3s
?v®Ù'¡à,?`óÜ÷3s
?ïuƒ/üo?'œoí
ËY?'Oš°Ö?'œoí
ËY?ïƒD\j(?¤§ïf¸m[?Ÿï—oKQ?¤§ïf¸m[?î˜e3'Ü? X(³mú0?®¶y­£¹D? X(³mú0?îŒ\ù;{è?–U†νŸ?§:0o·Ýw?–U†νŸ$AGN4FGL J2110.3+0808¿ "$ÐôîÀ9ëOÆðéÀ9ÌŤº_À<6ڇ s@Ò¡ÍðŽH@ÓÒåëÄ?¸r¹ÛÙZ$?²)°þe @?÷™DrØ@{Çb¦ÿ?ï1ž2°¿ä‹a'¦ãÚ¿å$†È½¯¿ânå€ÍÅÆ¿íKòa±ËÀ¿ÔOG› AGNfsrq3FGL J2110.0+0812PMN J2110+0810?ïûãê[å?3ÔãÔÓl±?@pVÍq‹.?3ÔãÔÓl±?ïçrgÑu~?k>âñ«Ä?h˜â/?k>âñ«Ä?ïâ"Ώ?m_ÆÜjF?mèã¥Ì˜Í?m_ÆÜjF?ïüÕ9ÿ?(âҚOÅÞ??9XÒ}[?(âҚOÅÞ?ïúíºÐm?@£ç·‡/?G´I
÷M?@£ç·‡/?ïxJ¤"ó'?—|rB?ö«m´?—|rB?ïÒ?œ'àW?~$mè©3?và1×\(?~$mè©3?ïö¶ˆÆ@I?BÎü¿''?R'îp¿½f?BÎü¿''AGN4FGL J2110.3+0404¿á=$Dœ«âÀ<@vžÂÎFÀ:œiW²n}À<T§i¦@  捓&
@>:}ªOÊ?È÷·1/"?¦FŒ~Õô?á6:Ÿ8?@©m˵u˜?ïî5!õÉ¿éV­@•ql¿à֋\¿ôw¿â:s™TÐ<¿×àcØl"¿é*''¥AGNbcu1FGL J2110.6+0403NVSS J211019+040418?ïû‰A÷`
?H8Z¾]E?AÚ÷aˆïÀ?H8Z¾]E?ïä2áö÷æ?}¤{Î¾/?kÍ$"ùâ?}¤{Î¾/?ïñߨ_?eÕm?%?]ÐBëÑð?eÕm?%?ïø\ü
	Ü?2Rq/où?NŒX•Z´?2Rq/où?ï÷–~ÔhÅ?MI|›*?PÓ¤%µÛ?MI|›*?² ?–¦E? é?ŽÐ{7½?–¦E? é?ïècmÚñJ?u'ýW¥t–?gœ'ã65?u'ýW¥t–?ïç8''¥û?WŠèg7:¸?hÇؾ<ý?WŠèg7:¸AGN4FGL J2112.7+0819¿á{ƒ<³jÀ:O9_JÀ9ìT3]û^À<%aþÈÈ@ 'òK—
?ü˜˜è™²?ÀüššËrÛ?Áƒœ—¥Î†@X¡ß¹8›@
,íZ`ô?±'l©¡y¿Ë¿ˆ®å±¿æi\ÜJ¿É ¹¿ú¿Ýù"ÏbÔ¿èîö«¢AGNbll3FGL J2112.7+08191RXS J211242.5+081831?ïþŠûNÈî?ÊN•ÖÀ½?'PJÿ¦‹·?ÊN•ÖÀ½?ïâ;µe?oê#&;?mÄîAF³L?oê#&;?ïë1ɞ™?p…
ûQ(Á?dÎ6yL¾¾?p…
ûQ(Á?ïðÚÌGtf?AA‹!œÿ?^JgìÉ"?AA‹!œÿ?ï÷Ñ1¿?KÝS¾<Û?P]鐢?KÝS¾<Û?ïadX—?œÓXàŸ?"ÓtýE ?œÓXàŸ?諾"$?ŠÍ~5€Ž‡?†¿ù/[?ŠÍ~5€Ž‡?ïχzÈm?d±ÿØ¹,?x<B¾{Q?d±ÿØ¹,AGN4FGL J2114.7+3130¿ëKˆ™c‹7À'ÄÂÖ©ÅaÀ9ïÉ¿Ò‡À<œšÕÚ@›`Ú5k@(Ç\Jƒ²?¾Œó$?¹&äàÎU?ú:bÒ]0@6~jê¿¿è÷›bFœ¿Ú¢^¤¦#¿äŽ	Bžá¿ßë‹Ô´ø›¿í.Œ¥•P_¿×®à}®¬AGNbcu3FGL J2114.7+3130B2 2112+31?ïô&EŠ‡?PûbÝÕé˜?W³t–gÑo?PûbÝÕé˜?ïÞÆ×P›?uåyéfe¯?pô­ÄΙ?uåyéfe¯?ï[ï~?‡À'	*?Œ©8‡«¼y?‡À'	*?ïÁëØß2^?cœƒ²"Aç?
"&(?cœƒ²"Aç?ïª-Ðó¢ú?'f›ˆc¾¥?…t‹ÍfW?'f›ˆc¾¥?ïEƒ'ßv{?¡­!¨õ–À?—O¥Èþ–?¡­!¨õ–À?î܄OÛ_?˜¶ÿjŠ¶?¢7»J5?˜¶ÿjŠ¶?î},</Ar?•cÒ:ßtÑ?¨-<;TÞ?•cÒ:ßtÑAGN4FGL J2114.8+2831?î!£ö¿èÀ+ϑ`4PÀ:-qRR³À;ØÔà—…@H'1·]@[˜fÙS?ÅóyÄ<0?¿Xòà\̊?öl¡«¶Ó@€?ƒ"´¶¿á·ü€Ä‹‹¿èú~¶¿D¿è•«}Ç«ü¿åtÞÏ-пïþÑÌæÎ?îU—¬Y¾AGNfsrqB2 2112+28B?ïýošÂ?.bv	Ï)?4ƒ0ASkê?.bv	Ï)?ïéß¼µõ½?n祤=">?f ClfZ¨?n祤=">?ïÚÞ+€¬?pqÕÔ&®?rêQÏ¡Û?pqÕÔ&®?ïû³N)6?3ˆÒ:?C©2!á*Ž?3ˆÒ:?ïü_¼Aÿ?EˆÞ#Ö¸€??5K4-^?EˆÞ#Ö¸€?ڬg?ž1>;yÿ?œIXUÚè?ž1>;yÿ?ïraŽæ7W?½½}^?'³Î&¨±?½½}^?ïÒ÷Ù7`·?jµæ)]Ó
?v""›øp?jµæ)]Ó
AGN4FGL J2114.8+2026?îɧëZÆ9À39"úÖËSÀ;
º(…ZGÀ<zÙ@x–@ wÅ3{X@qæ¤å'7?ÍĊÉr$`?§ë#$iî?Ýð¥dSÉ@	EíãðQ?ïÿàŠï²«¿éC_›q
.¿áÅÛAÖ¿áí6ß»¿ØV}JK¿ðAGNagnTXS 2112+202?ïÿ6"Å'?m߈ÎG?-ak–`?m߈ÎG?ï鸝bHl?n(ýû÷?fGb~,5?n(ýû÷?ï𮐙M?dÁäúه?^¢ßI™T?dÁäúه?ïýräpyÝ?ùüI"?4hÚi ­Ó?ùüI"?ïÿœF¶âo?	Ob};3Á?îEx5cï?	Ob};3Á?ï}—
o¢?Ÿ#ꄲpš?]Mš=Ï?Ÿ#ꄲpš?ïìöÕM¾"?oob2 2?c	*ðd?oob2 2?ïøšä?A"à–•‡?OúM'ž²?A"à–•‡AGN4FGL J2115.2+1218?ïhQúi#À8k•¢"À:B—Ò<èÀ<S‰®j7@ "¸ÌdÈ@B¡e?õ¹?·DʊRS࿘=~e¶"%?â5e<š»@w°˜¹ŸÉ¿Û9"5‰û¿ÙÏ~"DÎf¿æü€xá=¿ÏÔ<ãÚÛ¿èmH7§6:?ÏéÊÉàAGNbll3FGL J2115.2+1215NVSS J211522+121802?ïþ—üû, ?üñ+h•?&€-½æãç?üñ+h•?ïæQœ–?{uM\ó¬¦?i®ù//Þ4?{uM\ó¬¦?ïôFƸáˆ?^-‰kE>?Wrrj€ÿP?^-‰kE>?ïûh(ā?-"†óéK?A¾^¤62?-"†óéK?ïûÈ+ù?@Vó9eÏý?@ßS4†‡7?@Vó9eÏý?ïpÎ<õö?™íÛl /?'æ8]ÞeM?™íÛl /?ïë>¸€E?p5k5h?dÁG"†bÅ?p5k5h?ïðÀúS>?Q[`ùù?^~´—3|?Q[`ùùAGN4FGL J2115.4+2932?Öö"<vdÀ*¤$=Ìê)À89'T؟iÀ;u™ô2ld@î;'Ó+â@òŸYÌúð? ¼nþøå?»¤Ùh¼ü@Øú†C@Ѫc@l,?ïúû^Z©D¿ÞR%fÁÕù¿å7àAׁ¿ãùê<I\j¿éJߢ<€d¿î´ ~$É
AGNfsrq3FGL J2115.4+2933B2 2113+29?ï÷ûªöµ?K.TQ;?P¬k+¬?K.TQ;?ïÅA'MÅ?Ž.PÄj\þ?}tß3Ú]'?Ž.PÄj\þ?ï•,€H"?6E"è7•?Š´àõ?6E"è7•?ï÷;JÙÂÿ?@€*™xª?Q‰jZ8q?@€*™xª?ïì«âœlÞ?]B,i¥>?cT¥‹¢?]B,i¥>?îá?E:FÎ?°lW§gÕ«?¡ì¨ë÷(?°lW§gÕ«?ïié)òG?Ëx`zC\?'ÂÚÃv?Ëx`zC\?ïÞT›X?bH<ŒÊ?pÕü±Îè?bH<ŒÊAGN4FGL J2115.6-4938¿î¯N-4—ÀE®6Á]-À:­Y-˜¿À<œ™µHKÉ@.­f*+x?ÿPpûëžI?Æ<,9
ä?¶X|ÀÞ?ñZë­ó?÷<T "ž¿ß¶,A§j=¿çûš«'"¿Üˆ%=|7^¿Ý:ŽÜ§5d¿â\LœÄß¿è òž˜†õAGNbcuMRSS 235-024179?ïý:@È?3]ä$ʜô?6-ÿˆx)?3]ä$ʜô?ïåuŸ-F#?tD&ßN@?jŠ`¡?}1?tD&ßN@?ïí嗅(…?^Ì묶Õ?bhm~?^Ì묶Õ?ïáfÝã(7?T‰KeՂ?n™"\™ ?T‰KeՂ?ïü×e›Ô÷?5-/Ëw ?9DÒ2À6?5-/Ëw ?ïœ+žG?–‰û,`Ð?ˆùú.96H?–‰û,`Ð?ïíÄü•<?kVåúü!?b;áÍÐÛã?kVåúü!?ïIákH'?‡$°qIÚ?–ÃҖÿû?‡$°qIÚAGN4FGL J2115.8+6753¿ÞæY!³Ò@*	"ãÿïÀ;Dœ)¥ìÀ<"!É~c³@!m£4"‰?õÒ¼›&b?×u»Cš?ãӕsš+@ryJ@;íÞrÔ?àcƒ'«ìX¿ïÒ5A€R÷?áóRÝóe¾?ïÅèít¿ç&~"j]l¿Ýqü¼Ô‡+AGNbcuNVSS J211618+675324?ïôÇT_J5?N"ì>OdÆ?VqWO*O?N"ì>OdÆ?ïÅò€e–?ˆ§_ªàhá?}u†¼]™?ˆ§_ªàhá?ïˆO
!?†‡X@·>ì?ø¬=y÷Ø?†‡X@·>ì?ïb1XÆd?ƒç¶èo~?"¹ÔïÓY{?ƒç¶èo~?ïæ''çÎ?f…çY6?inسßbË?f…çY6?ïqc<ä?ªÔ}"óþ?Qӛ?ªÔ}"óþ?ï0ÑÆ£M?•ê‹W?4§?™åÇ5,^b?•ê‹W?4§?îvïUìNP?¢ýzÓPŒš?¨'
Ë?¢ýzÓPŒšAGN4FGL J2115.9-0113?ï¦Ç¢kzLÀ@'¼ÓZ…ˆÀ:M´ÒÛÇÀ<d•^¡v@Ng¹L½H?ÿùäwä=,?‡o vØy?ÀOâ€é'?û°ÔéÑÀR@šsPڎ¿ç*SÆP±É¿Ý‰å£©¿àâçÁDÙN¿ÜxwÀ«×4¿ïŒ~"ƒÕã?é³>¡%AGNbllNVSS J211603-010828?ïòxïL?aœ˜‹Ëÿ?[ÍÌí%'B?aœ˜‹Ëÿ?ïäî™dë?o²ØTÌRW?k쇗Tk?o²ØTÌRW?ï>Øfø¡V?¯!k4¬Z?˜$ó ëÕH?¯!k4¬Z?ïáV#Îo?Wí
øü¬•?n©ÜE-a-?Wí
øü¬•?ï«'ã–4W?†î™pìáœ?…6(1Z=?†î™pìáœ?ïcCÖ»ÛZ?—ºåšî?"—…%ø»?—ºåšî?ï*8"?"ß΀WÞv?Ÿ:°kZ<?"ß΀WÞv?ï\R¼Í?†?†vÓÑ?"}œ`4l?†?†vÓÑAGN4FGL J2116.2+3339¿Ò~5_ª­À%MOçžàÀ82LOcëbÀ;[í¤³©@¡Üí+g?ûòˆ-`‹[?¡Sʂo±i?¹.nRn÷@]Û	íÀ@¸Ü&$?æÇ·ÿá!C¿Ò½·†ªØ¿Ù"¾h…û¿ÙšÛ
,c¿âQßƤ•¿à`䡪µ AGNbll3FGL J2116.1+3339B2 2114+33?ïúÏ? "ã?I•
kÑMÓ?DÃ[Ö¹#?I•
kÑMÓ?aY.¬?‹iIˆC¸?€Ÿ©­%Ñ?‹iIˆC¸?ïÁt¡èr›?"I²ÊW?E¯$ƒâŠ?"I²ÊW?ïފ
ZË?Yž"êVD?pºÿæÊz?Yž"êVD?ï÷ËY–Z†?OžËfT¢?PiL"$%?OžËfT¢?îÈ¿ƒQóW?´Ä°º¼µ?£tÎPf'?´Ä°º¼µ?ïÕÛ:''×?ƒ+¬Éÿ•Z?ubӓÌ4?ƒ+¬Éÿ•Z?ï…Ò:Ü5?y£̯ޏ?Ž‹qV½"¡?y£̯ޏAGN4FGL J2116.3+1015¿ÏÌIôYoÀ9Ý˼+"ÙÀ:û,¨Õv¿À<e¯¶;Ð@ÇXÛch…?ðx
Oš?Ü¥0úØ#?ïÿì´É È@®-±éò@ƽñÿÁ·ù«
	¿ê
aw¤Q¿Õ©úºÆ»¿ëtÙé¿ïôL¾´ ?àV"Zî¹AGNbcu4C +10.65?ïÏÑŽ×?ŠŠQ&ß?x}?.à±?ŠŠQ&ß?ï¨nV¨`å?'Ö©–?…äj\Æþ¢?'Ö©–?íXŽ¿ÿg‡?¡&z#mԀ?µ;ŠàªÄ?¡&z#mԀ?ï[%õCJ?ƒâá}³0?"Ÿ=çúÍ?ƒâá}³0?ïöô5ÿ?¨ð­SjF?Ÿ!€<Ø!?¨ð­SjF?씥ʻ‹Ã?Ëä$?»ZѪ#¡è?Ëä$?ë€(Ê­€?­¹ùb6hã?Áÿ\ÕKª?­¹ùb6hã?î~e7V[?¥g+¼ªw?¨¬‹z!M?¥g+¼ªwAGN4FGL J2117.4+6159c?ïóWQºK°@!µo—g2À:²aç|À;ÔUÓq+¼@)Ñ,­Ýô@Ò¦-?Õɞoc?èÀ‰þ#r@
fr$àŠ@¼]Sm:k?ïþnÀ}>¿ÚkJw—¿ç<"Åý¦¿î-ë•å¯ó¿Ô}¢'¡Zƒ¿ï¡kTâ°dAGNbcuNVSS J211613+615920?ìŸ`ØTaÎ?½|{ªàÍ?»ù=\ñŒ?½|{ªàÍ?ç/£æ=zú?Êh5k-?Ñ ¸3…

?Êh5k-?ìfåׂ)Þ?¤˜é±ù§?¼ÈÑCî±?¤˜é±ù§?ëcuˉ*â?ªQWäØ?Âr(ÑÛTz?ªQWäØ?ç\…íÈÎn?ʅGTIЦ?ÑFô$nc$?ʅGTIЦ?ÀÂy±5±W?ƾC°aÆ?ëÏa"²"ª?ƾC°aÆ?áÚ#¨âÈô?º‹uX`ƒ?ÜK¸®:n?º‹uX`ƒ?͉8Çáo`?À6b½z?蝱Τ(?À6b½z MIXED4FGL J2117.8-1521¿îE;¯"¾ÐÀCp'IüÀ;Çwù5áÀ<hP?³t6@ÌYjÕa@ÏãzŽ;˜?Ñøòû4¿$?¥OiÒ~?̧Àä6Jë?û`¤$âãe¿Öa·˜ˆ¿Ýþ‰Î´¿à¶+ —ºœ¿çRÜ{–yT¿ïüt$•
¿?ï¶ý!ÿ.IAGNbcuTXS 2115-155?ïóõÐÒ?YÞ[îÒÖÞ?X]ÝdJ\?YÞ[îÒÖÞ?ïݗùí}ƒ?z¨m
ßò?q4èDþß?z¨m
ßò?ï_ nVí?­žÙÔ°?œTéži?­žÙÔ°?ïàwYRד?Y€(í—?oˆ¦­(l±?Y€(í—?ï읰ˆ&2?a¹íNf?cbOlÛ
Ã?a¹íNf?ï5ÑgU›?¦ áÞîµ?™EÓz£?¦ áÞîµ?îüÏó.­?"𽽜J|? 3ÎÖ'?"𽽜J|?îøªô_ãÀ?'ÅìmWðx? uP½q_ö?'ÅìmWðxAGN4FGL J2117.8-3243?ïÂHGu.ÀEïÚQÎÀ:z[ôœïÀ<M\ú¬Ùè@ ZÛ¯"«ï@eÏ?mÔ?½h"£¾5°¿šÀ>ÁS>c?ßX´Ae¥÷@ËÃw?ë€FvÜÖ/¿àÀÁü28¿äVóAUµ¿¿ät9Ûr­¿Íy¨7—¿ãý먰AGNbll3FGL J2118.0-3241NVSS J211754-324326?ï÷—B?E7<["fŸ?QÚÑ\¨qT?E7<["fŸ?ïèœÉÏÂK?p€ímè¤?gc5녅Í?p€ímè¤?ïÛqBþ?qâ¡3b¡??rrG=QÕ@?qâ¡3b¡??ïî{ô>‹?Gè­±Rbç?a"ÐE"?Gè­±Rbç?ïæYqC?`‹*(e)q?i¦Ž¾*æ?`‹*(e)q?ï"¢ùŒ?'I«úØv?Žþ—Këζ?'I«úØv?ïϝ¸žRÍ?|gp'£?x1#È3ñV?|gp'£?שׁ7»?uN"ȍë?"Õ{ϯZ?uN"ȍëAGN4FGL J2118.0+0019¿Ä\ñ— \[À?è">À:¥6nQsÀ<Wæ¯Ìâ@ø5˜hA2@ø'œ&;Ô?ÝíM
tÎ?ÚDôPÊ?ü@ÇÀôQv@SÐ|"`¿ßc[+J1¿ã­g¬·"¿æ*MçŸð¿ívjàžÏ¿è¦ÞHJG¿Àzz(ÓAGNfsrq3FGL J2118.4+0013PMN J2118+0013?ï÷*,é?s'F" ?QÑ«Š±"?s'F" ?ïëç^•Ùé?g<Eµ|³4?d¡‰Â~ó?g<Eµ|³4?ï[aÕÝí‡?Šªè
:Íy?""Å@Ò³5?Šªè
:Íy?ïùÍm0°?5sƒ1,°©?I¼ÊޒåÁ?5sƒ1,°©?ïø'¼–Úß?S–ĝíQ?Mµ
2;Ò?S–ĝíQ?/"(}?'1:ç[?ŠT4¨Ý?'1:ç[?ï€JŠŠ*?•®Rmž?Ÿïö°fˆÍ?•®Rmž?ïÞ{Åb,?c¶À¬
%·?pÂqUå?c¶À¬
%·AGN4FGL J2118.2+5752¿ïŸNPts@¹p]`-gÀ9Á;ϹçÀ;™j×o@àçñìA@	'C‰ÂŒ?Â>ˆ;xQ ?Ä}þ&×Z@TŸCý…Ò@˜öChµv?ï"]9–û¿çÖ´âË;Ó¿çtŸºšñ¿ç8×L''¿è©ç$f疿ï¾àÅýüAGNbcu3FGL J2118.3+575187GB 2116+5739?ï÷Äß1m$?JNÁ=Þé?PvA‡(7¶?JNÁ=Þé?ïêr9®L"?h3N"è?eÆc'sÕ?h3N"è?ïÊ´&sî?t•Ù±7Ì?zÀ%ûäPÆ?t•Ù±7Ì?ïäkÞe.?O¾0ì˜ý…?k"€,™'»?O¾0ì˜ý…?ïË2±@ø?yLbT	ú?zf§Ÿ+×Ý?yLbT	ú?ï9µÌç5?¥¢2kk‡?˜ÉFaa?¥¢2kk‡?íä1ÃF'4?¢náTÜ5?°ÞqçƒD^?¢náTÜ5?ïRH¤ßrí?€ª·ÌOp?•¶ëjðÚ`?€ª·ÌOpAGN4FGL J2118.8-0723c?ï¾D¤سÀBhß½jYÀ:ª(҇ ñÀ<,=]…@öE(þüË@8\gßã?ÍuÙ`ƒùI?Áޅ†è!?택Âô@¢ašú—¶¿æpoiDg8¿ån8¿,Ñ¿èëõÈ|Ü¿í†Ëá•[Ç¿îèïwòå¿ïÿüoQÇsAGNnlsy1TXS 2116-077?ïýsPY´§?4ˆIbR~˜?4e~'G?4ˆIbR~˜?ïçlêJG]?hݕYßhˆ?h"¡û?hݕYßhˆ?ï͸F"?x´†î~?y{£éˆN?x´†î~?ïñ}ïÖ?GþOÌ%÷?]çúÒ¥ô?GþOÌ%÷?ïû°
Qñ?Lãæ¤2å?A?Ö½»Æ?Lãæ¤2å?ï|Æf΍?"Ÿ0_ø?g3$v€0?"Ÿ0_ø?ïeï£fw?'1}étT9?"BŠš¿?'1}étT9?ï|'SgA?€ÎŸ=#P?ûJåÑ?€ÎŸ=#P AGN4FGL J2119.0-3317?äç SæÀFbMÒñªÀ;Ykã}é:À=!Iâ¢!@ÉH±Æj@ÃRë__?Õ.³R)˜?ïÔËi~K@ëÿÛk@ŸÖ
=UK¿î~ߧz®¿ØÌü½«FÀ?Û¤]Aúv¿æ¤Dî¿î1Ū™œ¿ïöF"¤ÐAGNbcu3FGL J2119.2-3313PMN J2118-3316?æch
õ$ô?ÊàCR7?Ó9/ä¶?ÊàCR7?ëúÈ{·äç?ÄÓóÌYÏ?ÀÞ le?ÄÓóÌYÏ?éÏÍwŠ?²6ە0Œ?ËüÀÊ#éÙ?²6ە0Œ?æÙ3Á?·¶ÜÕÁXž?ÓÜM™÷ô?·¶ÜÕÁXž?ÒoAT©P?͈o¬‹?æÈ_?U«X?͈o¬‹?âB	ÙXÝx?Ó[àI	þ?Û{ìMNE?Ó[àI	þ?Ô¥}R'r?Á±ÖãbK¶?å­AV·qÇ?Á±ÖãbK¶?Ó;ÿãí6?½àL	ݓ2?æbrŽ	e?½àL	ݓ2MIXED4FGL J2119.4+4652c¿Ò lȑdþ¿þ©Ü¨#$À;4ÒÆÒíÀ<¹?QN§@!~';ýP?ýBL
šµ?ÙzGĺ¯"?î£bۗjë@	÷ÿ=ba?óá–óÌëÖ¿ïøgàŽö}¿êæe$G?îÃ߈'3š?ÕW³%óà¿àb¥ç…µ·¿ïÿÿÊPËAGNbcuNVSS J211922+465026?ï­Vê6Y?Œ½z*x?"¼êEriÄ?Œ½z*x?â}ñ ŸOð?Ñ'æÝÞÜ´?Û¾Á`!?Ñ'æÝÞÜ´?î¯ÎàUô1?—M&͔àÝ?¥÷1 ö?—M&͔àÝ?á¸ë«¬Ž
?»µ]‹—M?܎(¨¦ãë?»µ]‹—M?ïžÅͪ?›x$´?ˆ~¿Ñü1u?›x$´?ΚòiêTr?ÐO¨Š°?èYCe…jã?ÐO¨Š°?íôùg=.'?¡G~€ÏÎS?°X4Ä^½p?¡G~€ÏÎS?Ƀ½5i@?ÁD֓õëª?韲»å°?ÁD֓õëª MIXED4FGL J2119.6-1105¿ç¢·æ
áÀBñŒ~($À:oÍuhÀ<KÛ$~dŠ@9"v¢s³@þZäR%?»§!	K>?³Ó}kÃl?õN¨‰÷e'@édZ&?ïìpk¢æI¿çóZ4ÿ¼
¿á¶ôžM›¿ä~q f¿ç™ÌYàF&¿ïïÀý¶¤—AGNfsrqPKS 2116-11?ïý¼÷Ë0É?6½Å¼7³?2B:DE?6½Å¼7³?ïíÀÝÖ4€?fRÛ¤Àæþ?b?"툊?fRÛ¤Àæþ?ïà¯jÓ?pü_ž¸r¼?oP–JN?pü_ž¸r¼?ïÿŽ­E?
˜X˜`6?"‹zÜè?
˜X˜`6?ïûþ?EŒê-"ì?CƒîûhMô?EŒê-"ì?ï¨ìNXŽÉ?‰ÀU¶Žô"?…Äìt+!Ì?‰ÀU¶Žô"?ï—…áo¶?‹µd_Ø?Š8Þ}U>—?‹µd_Ø?ïþƒ
¶è4?ŸÂ™‹ƒ¯?'ÏRÅC?ŸÂ™‹ƒ¯AGN4FGL J2120.6-1254?í'*)Á'ÀCnş±áÀ:hß۝J(À<d×ؙŠ@ÁÊÍC?E@}!xö‹ã?ÀÍßÇPa?®Â_œ®Þ?ìܙÿ&ó@€×€ÚÜ¿åîO¾Úé¿ÑŽ)ùΎ¿çñÝþMx¿áõ!HÏþ¿êŸåãõ~¿ÓUžã/»AGNbcu3FGL J2120.4-1256NVSS J212035-125443?ïü«¶§œ?.³Aš¸³?9ê¢Ruoó?.³Aš¸³?ïìÁ "•Á?gÍLžœ^?c>߅'nô?gÍLžœ^?ïá@$èJ?e­ö ÄÍÐ?n¿èÉ9½¹?e­ö ÄÍÐ?ïü'͸Ó?$Xf<É+?;q•Ü¨\­?$Xf<É+?ïõü&_Bä?M«¹ß}—?T³.<g³?M«¹ß}—?ï¤N7ÙU?ŒØ²ó­˜F?†ìr<ZÄ?ŒØ²ó­˜F?ïÙE³cq?y¶N{y :?s]&w¿#t?y¶N{y :?ïòÌm×Hý?M
Û¹&Ӟ?Zg$ôç?M
Û¹&ӞAGN4FGL J2120.6-6114?ëÄ»m¡:šÀDžî|IýzÀ;!—rwíÀ<¸£ûó+@OYýÍK@/ªJè\?Ð/níôdÁ?ȑòƱ¿?ölaR*o@œ7^+œ?î]ÝÙ¥¿å‰ÚÔ¯¿ã¡Œý©äj¿äsƒðºèŸ¿ä¼27Š±¿ïþ N¿€´AGNfsrqPMN J2121-6111?ïýS%I™/?.\#žE°?5fÕä°é¡?.\#žE°?ïõ"áÆP~?Y…±¬Ì+†?TÖ;ò-´5?Y…±¬Ì+†?ïèÍÆ?\×&ª}.a?gb3óm?\×&ª}.a?ïûÒä­®?'M¬ù£:œ?C¬´9›õw?'M¬ù£:œ?ïþ–]úÝ?"õ"¤ä¼³?&š!xÛCÊ?"õ"¤ä¼³?ïÛ-•0ö?vU…õK;Ö?ri5IH(z?vU…õK;Ö?ïÐuŠv?y`"¤ú†©?wÅ;Y|œ?y`"¤ú†©?ïëÔ`%?ç?Rf}‰Tê?d+ 
Ú¡?Rf}‰TêAGN4FGL J2120.7+4428?î_ff€+xÀ<AÏ®)À:?±~'­À;¨iTWp)@æµ+E~@Q*Dw(V?ÇI/ôºQ ?¡M¾ú§%ž?ÚiœÁAS@d‰ÉAþ?ïþj~£ôç¿á+"}¨¢K¿ëáxU|¿á2Åð9¹_¿æyÂr«Ä¿ïÿîbHÊtAGNbcuB3 2118+443?ïõ™BÂÙj?Tå÷ö3?TÍz…Kë¦?Tå÷ö3?ïàÚðÉM´?vñµñ[Oñ?o%•Dp?vñµñ[Oñ?ï€J}k?‹"]·'?ú-VpD?‹"]·'?ïØì7B®É?V¦ ˜€Z?s‰äo&»˜?V¦ ˜€Z?ïÆyÒåü°?¥ú?ì"?|È24?¥ú?ì"?ïnôŒPÓ$?œœdô"1?'!nwiŠ?œœdô"1?íî›Û'!?¤EôQ¼"?°‹!%9s?¤EôQ¼"?îé+DÒB?‹ÚI}›ð?¡mK±ÿøæ?‹ÚI}›ðAGN4FGL J2121.0+1901?ï´YIiÎÀ5>
 r~À8Šr©jÇõÀ;£ÊÖR‡Œ@¤Î(š@>Õ®Þ]?¢^/š;?­c|ö÷@ÞZ"Ê@
yñßÖ¿À?³mÖVοá÷u¢™r'¿ã‰-°ê¿á|¾ß¤@¿æóBýօ¿ëM³"íbAGNfsrq3FGL J2121.0+1901OX 131?ïýMÔÛJO?-¢
0Ù7+?5'ZK?Wž?-¢
0Ù7+?ïÏqÔrw[?›½?£õa?xG禇?›½?£õa?ï¿JõQ?†+2ß?€-BÃõéÌ?†+2ß?ïžô½±§?pÅgýçO?ˆBú^R7?pÅgýçO?ï÷gñ^…$?QÉþ^eÌ?Q0Bõ·Á?QÉþ^eÌ?îÖJ*Äø?®`§G"?¢›]S˜-‰?®`§G"?ï®ãyڞ?ˆ_®X›â?"G9×êp¢?ˆ_®X›â?îBøS.?•þ'(\a?«ÐzÍÃÆ(?•þ'(\aAGN4FGL J2123.6+0535?¿7|Õ#ðÀ>µÜyÀ9é't1*DÀ<6¶NÜ&@½'ãɾz@
b*Vì?´+®À®l¡?"plN²À‡?àFǨ ž@
ònòÑï? œƒ¿â¨b8Yc¿èž»ýq°G¿â´ˆ"MÝ®¿áØ­«ŸU›¿ïÿânÁŒAGNfsrq3FGL J2123.6+0533OX 036?ïýK†Lq?/WPŽ?5£Ï'ñø4?/WPŽ?ï瘂9Íù?{{	ï~?hg}Ǒޔ?{{	ï~?ïí|0j?hëÏ(H?bþ"«
a?hëÏ(H?ïù+ŠRa?5:Çõìð?KQÕ­å¯×?5:Çõìð?ïû;!ê
 ?C&l1!ì?Cy'dd?C&l1!ì?ïŽüª"?"cË®é?Œ@Õx¼+?"cË®é?ïÊéí2âš?€C
qîæ?z‹	€«ºÅ?€C
qîæ?ïìۺȵ³?QAz€^"?c$Dü1?QAz€^"AGN4FGL J2123.8-3148?Æ»ú.QCŒÀFæÄŗNÀ:µkÞuk½À<KŠ·~‡@Ï¡ê ó*@™cˆÕý?Ô]•\s"?à¿-§Ø÷}@0[b&eÅ@^lg1g¿æ"íٌÏ?ïçô÷í¿ë/•XÆ¿ç2UB&Á
¿ïîû.	(¿ìZVÆy÷AGNbcuPMN J2123-3155?ïÉ¡uÊÌ0?}rJYY?{/E/ç{³?}rJYY?ï)Ôr(^?­tÓ1Wö=?šÅ|6â^<?­tÓ1Wö=?î
	A$ëû?›îApö~?¯_kí±@L?›îApö~?îöj'²L?†²¯j;]#? ™V&øô:?†²¯j;]#?îɲ–à?«lဓ,P?£nDÝ"Ý?«lဓ,P?êíŸ.Ãs?É]€}'¦}?ÄIƒÓDò4?É]€}'¦}?ì@ÈáÊz?¨5å''/q?¿Ýù¸ñ¬3?¨5å''/q?ê<;3v"Ê?µxc(™QJ?Ç2%°Ø?µxc(™QJAGN4FGL J2126.1-3922¿ïç†p‹ÈÀFþ"ž­Õ'À:µ~Ư|ZÀ<"ú~Ù@ÕôÜ5uƒ@™ñ®-¥?¼A<á1ޟ¿£²€f­?çÀŒ¢8G@!ýŽ?ïý¸ýâïN¿ØL9)y¿¿çê¹aµý}¿áY3BL«ª¿ãùïzv¾£¿Ò<ªÏ'AGNbll3FGL J2126.5-3926PMN J2126-3921?ïчƒ?ĸoÕrZ2?Ÿ%ß0Ô=—?ĸoÕrZ2?ïétgÿ?p€ÛÂf÷ñ?fç‹M|8Î?p€ÛÂf÷ñ?ïƒD{–?2Ÿ°!)ø?.áIÆ­?2Ÿ°!)ø?ï÷7WbÅû?5§øfDw?Q'PÄAy¤?5§øfDw?ïöº#`?^m#ñÅ×?Sҋ‡ñ'?^m#ñÅ×?ïEÂ/̺?¥È®yz^?—Gº(³?¥È®yz^?ïn`õ}	?•J|×À<?'3áU†Iz?•J|×À<?ïÙþ½FT?_ÒÉp^ÓC?s¡vkñÝ?_ÒÉp^ÓCAGN4FGL J2126.3-4605¿ÄSš7_xóÀFÏG0@9¬À9kæ'øÀ<5/Ùâ_@\XúÂÿD@Aà?pXX?¦ó5—;›b?¥P(as'?õõ+á/Za@Àw¥("¿ÍßÈýà@¿ä/D%ɾ%¿èèSpÀ\|¿ãOCÕAæT¿ë`›KJ.¿ïúÕô"»3AGNFSRQ3FGL J2126.5-4605PKS 2123-463?ïþŒå^È?&¤y)?/§4Ùéõ"?&¤y)?ïõñ.?Z	ªSu?T£²×Ã?Z	ªSu?ïк^¤êÊ?xùWŽ—?w¢Ðî3?xùWŽ—?ïÿö-Õa'>Ìè>Ó¤Ö=¼>Ìè?ïÿNÀ5m?€Äµ%a?'ý¡‹÷ö?€Äµ%a?ïÝùÜ`¤Â?tI"rŽæ?q°Á#W?tI"rŽæ?ïÛƒ0ª?w¡‰ûàlW?rw¾^ê+
?w¡‰ûàlW?ïÿõX²Ê>ÕÈҎÞÊ>ÕNÉ«L"Y>ÕÈҎÞÊAGN4FGL J2126.5+1842?摩ڞ5yÀ6m»{k±)À:ÏáÕr¼À<wª¥æ¯@ 4‡†Êµ@ÛÄÒ,ˆ?Á"AÞÇ¡¿¢|ÉCI?äMÝ|è‰@aŠžÿßõ¿ëä¡Ý4ú?ïÿÁeÖt¿êÁj=¶nç¿ÉŁÿÉú5¿á*«ýI¿àaO`eprAGNbcu87GB 212407.5+182753?ïþj&—÷â?m³IúÖ?)]™Ê»¼÷?m³IúÖ?ïçB…ûEö?m±5.Ål/?h½yߞBl?m±5.Ål/?ïãfHÖªé?tºf'4R?l™¶ë|æ?tºf'4R?ï÷æTn}r?4×£MÄD?P3Vî>NÍ?4×£MÄD?ï÷É™<?P+p…Û|?PmÊàÅÇZ?P+p…Û|?ïfĎK? 4_±€?"'n3-aµ? 4_±€?ï×G1b;?} ºù?t\gi°šª?} ºù?ïÕ2fÚ"?häҌ†4?ufÌpdÁ?häҌ†4AGN4FGL J2127.6-5959¿À¡ÚSŒßÀE=¿H˒À;X?½…1-À<Üdçá%I@ š-hC
l?üuãTΎ?Ë:'C:è?ÃÃú€º$ª?÷ځNš@""¯ ê?ïîy$¯ò¿í:䜸2?ސ'¡»ý¿àʐ¢Oοåñ6;%¿Ñ²'¤\ìAGNbcu3FGL J2127.5-6001NGC 7059?ïýî¬+Óª?'*ȓÿo?0Š ;€Ý³?'*ȓÿo?ïóù݄³Œ?]Ì	Ø?Ín?XET׫?]Ì	Ø?Ín?ïçےH¨¢?ož¾å`þ?h$mèѾ6?ož¾å`þ?ïñJ@H£?Fi$"•?]kt?Fi$"•?ïüƒÿS‡¼?4Qk4b¯>?;àÛʍn?4Qk4b¯>?ïÔëüVÁò?x®ûª Â?uŠÆà–Ý?x®ûª Â?ïÌRÆ?Ñ\fÐÉý?yö֐aãÓ?Ñ\fÐÉý?ïØæ×B¥?ei×ü€ ?sŒ"gœl–?ei×ü€ AGN4FGL J2127.7+3612¿¹AlÀ%ùÁø]tÀ9Mo«‰†&À;ËüÞ1@Ês×K?üþ_·¼^?²a>‰R¥?ÀN®ä¯l•@¨!ò™0@1<ëج¿ÎÍÅÆ[¿Ùú$‰LD|¿Ø~¤`GŽ¿ßŽ?ÒþÀ¿Þ4"ý#Ö¿ëá& þ'ÃAGNbll3FGL J2127.7+3612B2 2125+35?ïü¶ÑÛ ð?4ò¼[Þ-E?:IqœžS¯?4ò¼[Þ-E?ïÝøe¤A
?uãã i
«?qÍã;B?uãã i
«?ïÙšRx?v[!×Eœ?su²ÛKÂ?v[!×Eœ?ïïÀï7ʋ?AqƁÝ!ó?`?Äì˜?AqƁÝ!ó?ïõTßðø?RÑaÑë?UV@goï?RÑaÑë?ïW¹5§gõ?¡&Ra7,±?•ÙB{ûy?¡&Ra7,±?ïªè3FS?ŠëQ2§»ÿ?…E߬O3,?ŠëQ2§»ÿ?ïÂÄp\ßT?gmÜûŽÄ8?~ÇÉQF?gmÜûŽÄ8AGN4FGL J2130.2-7320?±ÕÖ՜ü'ÀBmß 'áÀ;JòÌ:֖À<Äô,'@É{ôíþ ?ý=¨!ò™?ÒáÍdø'D?Ԋ\¥Gw¹?ø*²ái<@8ô‹(?î˜32\sž¿íè†1		?²|Ç£m-¿ækµÆ 
b¿é/ôq¬¿¼%p§ÝÕAGNbllPMN J2130-7325?ïö»˜ûm?K¢ÿfMÅ/?Sîˆú&w?K¢ÿfMÅ/?ïóæéó=?]Oó­=¼?YÀ2)YÕÞ?]Oó­=¼?ï¬^ûÿ?z´gö"U—?"èAE»84?z´gö"U—?ïñcOZ±&?DêçÐYȯ?]9aR'?DêçÐYȯ?ïè9ª/$?cJò;ÌÌ?gÆVíãß?cJò;ÌÌ?ïÖÖË÷K?M½­]?t"ú&bòi?M½­]?îê+7;U—?•ÄgǑ-ø?¡]LºB"?•ÄgǑ-ø?ïÒµFÉ= ?gÛ- :µ@?v¥\ze0
?gÛ- :µ@AGN4FGL J2130.4-4241?ï(·ëPÀGUž™ À:•êњ'çÀ<t&"»@G6¢0—@Ð#éê?Æ?a>ß8à?›ÕW	ý?ø§°³'@Ù{´Qy¿éæÍÿÒ³—¿Ö"š.¿çå¢'<¿ã8?ân¿ïû›÷Ì«¿ï=I6ª·AGNbcu3FGL J2130.4-4237SUMSS J213017-424319?ïÿ)¸Fi?˜A¯·Þ?šÎö9?˜A¯·Þ?ïö"–$f‰?WòqB&±ì?SºÔèQ?WòqB&±ì?ï¿YÖfI?¿Jk#³?€)Šp7qÆ?¿Jk#³?ïÿê
¥Z>Üt¹lf>åò€Âk@>Üt¹lf?ïÿ6iH˜ö? 0å•Y²á?2ÏïÁ*F? 0å•Y²á?ïØ•H7b?]zÎQ®?sñµJ¶BÙ?]zÎQ®?ï¦gòè¡?‡$sw§ô?†f…"«¨?‡$sw§ô?ïÿϲÊ
>òô3è¤p—>ø&ˆó±ñ>òô3è¤p—AGN4FGL J2130.8-6623?ïü‰•ŒæûÀD È`VíÀ:@.A[êâÀ<Äa¢—o@1O¥"´Z?üØ´|sîå?À'ý]¹C®?ähY …F%@ }(®tòñ@ÿ9Cm"¿é Û!¤??êìȀ6ò¿Ò//bÄw¿é.äïÙA¿ín—ø¯©¦¿ïýÑò¦{)AGNbcu3FGL J2131.1-6625SUMSS J213038-662356?›#¥nŽ'?ªèx瘊?ï&âԏӌ?ªèx瘊?Ò	"mã]]?Å×dD<	?æû=ÉQR?Å×dD<	?ÄÀqñE8U?¬WPõ?êÏヮ±ë?¬WPõ?Õ/?õ?¶E‰Ú±R?åôè}`?¶E‰Ú±R?àý…ûÒ?ŠPdÃ_Í?ïÀ>â+È?ŠPdÃ_Í?²é"ÝúÍ?´f{˜;p{?í¢ÍdCÃÇ?´f{˜;p{?§>Ù&åÌ?›ÝЌ<<[?îŒmžq£?›ÝЌ<<[?›‰âö¼?!‡ê8¦6?ï#³'ŠÂ?!‡ê8¦6PSR4FGL J2131.0-2746?ÚlEØD$ÀFì×à&EåÀ9‹‡T¸À;ìh?"zN@3úÑíÈñ?ùóúˆÇº>?²¼;7ó?¿	Hþ÷l^@+ý´Ì%@
§&5ô®"?ï'v Ùó?ÁDµüü•g¿ÉΆö©À¿ÜZŽâ™¿ØÇÓ~AÏX¿ãcs¢¡AGNbll3FGL J2130.8-2745RBS 1751?ïû_MÝj?AŸpàÝ?B'Èv"Ë?AŸpàÝ?ïÚÁ9<»?ìðÚLU?rŸc~pƁ?ìðÚLU?ï¥Ñ}zn?†³]Ï2?†»‹–R'?†³]Ï2?ïÐN±‹JC?`VýEn&Ø?wا í°?`VýEn&Ø?ïãmÒZD3?lÉy&Ë+?l'-ؖÀ?lÉy&Ë+?ï5ª½y?¦þE|ñI?œyJ¼PÔ?¦þE|ñI?ï'ý`	øI?±w0ãø?‹€§ö¢µ×?±w0ãø?ïgÉê¢Ô?'ÏÒ#ÅuI?"ÆAu?'ÏÒ#ÅuIAGN4FGL J2131.5-0916?ïэ¾fyÿÀCÖ@|ÇÑ»À9¥
œ;5À<%Åo@	_	ç?ÿÃnÙј?°gÆä*Œ?fœÏŸ‰'?¹ìÒў˜²@
-:×ÂI;?ïsÿi­¿ßD¦âÔ¿ãÿ•g0¿ÚE¿'Q¦¼¿á•Ÿ¤u•®¿ÇôwáùþAGNbll3FGL J2131.5-0915RBS 1752?ïþ.³éôG? @Û¤»ŠÍ?-ÀÆÍ? @Û¤»ŠÍ?ïî>bc?dbuû"…?aÁª"}E?dbuû"…?ïõc)£›?G˜¨°}?U9¬2K	?G˜¨°}?ïû"}c?0@>ý%=Ý?A³ñ't½?0@>ý%=Ý?ïüÕEæ?1',RO$?9W/ÇWê»?1',RO$?ï '|¾?ŽÛ¥À‰ì?‡ö ɝD(?ŽÛ¥À‰ì?ïñBtf&?f•«ÎÿoË?]ÙzÊ<tÞ?f•«ÎÿoË?ïø½ëÕÈì?=W¶å9,?MO§mK?=W¶å9,AGN4FGL J2131.7-2515¿€ÏQ-çfÀF»F^‰"SÀ:YìÝ
Œ°À<ZSÆP±É@ nYÎÓb=?ûÈF¥Ö¾¾?À¸ô'ڏƒ?¿×´ÝAäý@ÅzxQJ@iÂß84O¿ïŽI9.õ·?ê)¯[¢¾¿ÙÁa3Ϳע."'AÜ¿àÿŸY¿ÕŸç't1AGNbll3FGL J2131.8-2516RBS 1755?ïü…lïu!?HCWÕbb?;Ԙ'ˆ«'?HCWÕbb?ïß3q
?}ªŸ`åìV?pfGè5?}ªŸ`åìV?ïê$º'6X?cØ¥ÂÓj?eÛF¥i?cØ¥ÂÓj?ïÕÊ&1?YºÔžÈ˜Ž?uv0w"?YºÔžÈ˜Ž?ïﲋûC?fùŠDbí¢?`ëM"¡%?fùŠDbí¢?ïK}	'"?£i‡ýÁ¬?–^åòd?£i‡ýÁ¬?ïË3b-Â?Áˆh÷<Æ?zfNûPè?Áˆh÷<Æ?ïO$e£j?…kn( ´Ë?–lXrü°?…kn( ´ËAGN4FGL J2132.0-5418¿ëp´7¡úÀFliƒQX¸À:	²Œ¯¦KÀ<jńÙîô@Mä@Ü¿@G?Y²#?¸y€Ÿwª?³ƒS‡ªó?ø9ߊ>²Ã@ó–ßU§?î+|…Œœ[¿áEäEVJ¿ä^_[Û¿æIøÜö¼¿èñÒÀ¬­ó¿á_L@ËLDAGNbcu3FGL J2132.4-5420PMN J2132-5420?ïü`|Tv?cqtÑ×?<ÿN$T"?cqtÑ×?ïöä/acë?WõøÔ½/?R7 ÔÄŒ?WõøÔ½/?ïë PºO?YwÐFØð/?dà_žÇ'?YwÐFØð/?ïýú1½oë?¢ëNÉÔF?0.qWbô"?¢ëNÉÔF?ïû3ù	tQ??|B]ñ?C0P"å??|B]ñ?ïٞ×,?€3+pÝù?s0ù§MÒ?€3+pÝù?ïÎڎßßØ?}t†o\Ë?x'¸£Mä?}t†o\Ë?ïú;ÎÅî?9E'ç?G¥h/R?9E'çAGN4FGL J2133.0+2610?ÁA¹DõÀ2q»à~íÀ:×Üßi‡ƒÀ<?‰›ár@ù¨çj\ë@¯ŠÄê€<?˯æ8óg?Ör$u*Nˆ@ýæJLT@´²@¦(?Ñ
8þyB6¿â¨˜é_¿çMFkE¿äã¼gú»¿ïþ€¢§µ¿±Y¯ô¤ØAGNbcu3FGL J2131.5+2605NVSS J213252+261143?îø/!^R#?´Á™…%-? }
ècÌ?´Á™…%-?ìÂÐõ{l³?»Ýwâ1/?¹éxT$ši?»Ýwâ1/?îdT"
"^?—ó½ò?©º½ÞJã#?—ó½ò?í¼ñ½>†Æ?¶}dö?²rÖR?¶}dö?î4Ï+»‰r?¨ ôÖÆ?¬³
BšÞ?¨ ôÖÆ?Õ,·ŽL3Š?ÐjË͕Áë?åi¤8Ùæ;?ÐjË͕Áë?é–u$¢Õ?±S´§ÏØ¿?ɧš+mt«?±S´§ÏØ¿?ÚCóý4Àô?µmf³-ãj?âÞeŸ†?µmf³-ãjMIXED4FGL J2133.1+2529c?⸷äÞ;ŠÀ2óNe¾ ºÀ:«ï}Ѽ÷À<j"l
ë@ ¬³Ho-?þȼg#ûˆ?Å'Pǘ°?¤Pl ‡‡?ã>Ÿ&Kn@û©Ã2o>?ïúޝڛí¿×Ô¿?E-¿à£^Caÿ¿ÎR$zˆ²A¿æ»Ê`áÂ'¿ÒƒSœŠ9ÕAGNbll3FGL J2133.3+253387GB 213100.1+251534?ïþÈäϑ½?DFé[?#q³lã¤?DFé[?ïî€9(ô?e´N0y—^?aƖs:²?e´N0y—^?ïõÌZ¢>?aÃÚjg?TgKý{3²?aÃÚjg?ïñ
<€?@ÿ‹_!
?]óëêˆ@I?@ÿ‹_!
?ïü‡ïr&?<ÃéeôØ?;À†µ¦N?<ÃéeôØ?ïŠL虏'?—iP6àM?lÅÖ,·?—iP6àM?ïôÝû¦Ýƒ?f'«÷fÀ?VDé>º©?f'«÷fÀ?ïÖrŠX€l?`¢•SRO;?tƺÏ?`¢•SRO; AGN4FGL J2133.6+1439?Ïë$¾GÆ5À:d6†¤ÊOÀ:½|·¸À<" ()ö@@Ã]NÞ@ךCÅ
?Æü7ž}¿®$=®X»?äµÎMÖL¨@c']çç°¿âøâÕLοë]
Œ°}¿å'z¡0ç©¿æ9Mß0ýy¿ïæ¸f
{¿ïÿò> wAGNbcuMG1 J213339+1443?ïüwˆUW?@Ôé´~Š??$A¤Å|Ü?@Ôé´~Š?ïér²¥Z?h&R`[E²?fMCŸMù?h&R`[E²?ïÚD‰iB0?v©Ö'u«?rÝ»YWÉ?v©Ö'u«?ïù±ÐOÁ½?4Fþ'Ô§·?I8¿¥«Ø4?4Fþ'Ô§·?ïýÙíq²ö?9­Ãe/×?10"0@'A?9­Ãe/×?ï'ôgþ}?–.þH¯l?BüðO4¦?–.þH¯l?ïږR×H?{£H\À´?r´Öª|Ûë?{£H\À´?ïÈ´žF–V?o8²üÿˆù?{¥°»¸•?o8²üÿˆùAGN4FGL J2133.9+6646¿¯ïg_g¿@%ù
{é…jÀ9Wòw@ÝÀ;òd\ êÇ@åÄ[º@èà(Ê$?´"54Y©?µ@b›«—ž@
Ú\ˆ–@½"NXӁ¿â<kU¹où¿Ñ´ådô y¿ån oQ¿Ö'°œ?':¿äé2(q8R¿åFÆÞvB|AGNbll3FGL J2133.8+6648NVSS J213349+664706?ïý¨Iµ«ž?^÷Ïÿ'?2½°[…þ?^÷Ïÿ'?ïï'óÿ…v?d¢mF`&Ó?`}â=ú›?d¢mF`&Ó?ïôbûe3?cȀŒÊ·?W;Â50™¿?cȀŒÊ·?ïô±Ê+Ì{?@R%òSÑ?Vœk$v	ý?@R%òSÑ?ïþ~±>"~?î›"n?(ê/‰A,?î›"n?7¥M?š'6w'?‰œ¼e€Ë?š'6w'?ïð`©Ÿ1?p¼øÖ*mŒ?_Á>>κ?p¼øÖ*mŒ?ïÚÓ2ˆ?b(ÂÌ*Öç?r–fߊ ?b(ÂÌ*ÖçAGN4FGL J2134.2-0154¿àÛy"À†ÀBDzd×ñÀ9àR»Ž·À<I—"Ç@Ò¤e¥vG@DfBT?ªýd©g?«èž ¥¸@=ÙÂ~•1@‹–'(6*¿ÖóünñO¿ãaþ»Ý;¿äîvjÀh:¿â#•›Þx¿è • ãû=¿âᙹzAGNbll3FGL J2134.1-0152PKS 2131-021?ïý÷hƁÉ?'(±j`<?0D¹§©"?'(±j`<?ïì	%÷%?gåJîÍêå?cöÚJåZ¦?gåJîÍêå?ïéÉIö‡?n½ÿß±œi?f6¶V.?n½ÿß±œi?ïý˜ctÖ?)2Ÿ'_¿U?7;>;e"&?)2Ÿ'_¿U?ïûðVI…?7Üv)ËÊ?@?‹ŸWC¦?7Üv)ËÊ?ïE	õLH?'‹éj­Áñ?Œ.½=R?'‹éj­Áñ?ïÍFZékÐ?}úDŠŒ¡?y\Ҟ‡çÙ?}úDŠŒ¡?ïùÀ:Ãz??+͘äÏ?Hÿ?ì›??+͘äÏAGN4FGL J2134.3-6511?ؤƒ6D¤dÀDc¡À:Ç+×_gÀ<aýõ}Æ@Zt¥™W@Cá8j«?Ðe¦Ñ?•ÿ¥DÑó?·™¿¯,þ¼@ª7îý`¿ìÒÿõ5¿åk›#ÝTÚ¿àm>K?D¿åNìóà¿å°¨t'ð	¿ïîW–¿Ê†AGNbcu2FGL J2134.5-6513PKS 2130-654?ïþö
ë²?ü9='*»? Ÿ\#@'Q?ü9='*»?ï÷#1!Nô?Tl"ýØËÅ?Q¹A°(Æ?Tl"ýØËÅ?ïðµ`ä58?cü>UÙVð?^•>01?cü>UÙVð?ïþ,3ö¸À?p¯¬Ó¦"?-<Â[¦¨'?p¯¬Ó¦"?ïþaZkŽø?%ܟdån[?)ê\Ü£"?%ܟdån[?ïÖ{s¡&?"K(‰c1?tÂ}@ æ?"K(‰c1?ïê•N§û?p§~xoÂ?ejæv>½)?p§~xoÂ?ï÷o'pA?EqH©w?Pý W.5?EqH©wAGN4FGL J2134.5-2130¿ét}JÀF‰Mçê_…À9xˆ3?ÈÀ<¸_W~l@†Cmqs?þÙ²"ý[
?°Ï¹Wf?²Gšs^F‡@¨Ÿr÷@)0Ôßù¿ïëC_Ñ ï?ïÂîþGn¿Þ¨èèŒF¿àcª2n¿á½?[_¢'¿à*MTAGNbll3FGL J2134.5-2131NVSS J213430-213032?ïþ°Ä¥Ù:?CçÝSã¼?$ó²y.Äm?CçÝSã¼?ïìžÔ®?k[Hc·?c=afú™d?k[Hc·?ïìj·âb"?a‹þ{Ȅ³?c•H?ùƒÿ?a‹þ{Ȅ³?ïö‹ýϤ?>ê¼]¼3?Rèá+?>ê¼]¼3?ïüáÞ½÷-?1Ú,‹?8ñ
EVz?1Ú,‹?ïo×Ô<Ù?'I\Y6?ˆ¤
?É?'I\Y6?ïØ´Æß?xi|hÙ¿?s¥œöˆ†?xi|hÙ¿?ïçI&~]Ã?^¼ûYm?h¶ÙdŅe?^¼ûYmAGN4FGL J2135.3-5006¿ØcF'FÐ/ÀG3)¡¹ù‹À9-w9ó@ÕÀ<AÞÌ©'^@])DÇÛ @'bå¨eå?¨µ#§"Ç?²Ë›^ëÈ@"˹§V@_kó™d¿Ðð÷¹à`þ¿áîÅæ(¾e¿æÔ²¡¨\¿å§­ÞÊü¿çȈd½ïº¿íÃz=³¿¶AGNfsrq3FGL J2135.3-5008PMN J2135-5006?ïþáÒøc?z.†?!âÞzñ:"?z.†?ïö%ñà"?Wà+ü>ž±?Sµ×Á‰)	?Wà+ü>ž±?ïìØäï>£?fIv\ éå?c'`E?fIv\ éå?ïüÅÑð‰?,^µº$2k?9×wYe/?,^µº$2k?ïÿ¤yá1?8ÃWÔP?hÂ\{$?8ÃWÔP?ïÝ}¿?sà
¢"$Ó?q@s­2½ì?sà
¢"$Ó?ïåB¦‡'…?pˆ9¦f	?j½Y§8+&?pˆ9¦f	?ïõlzkoÔ?N…$Yµ?U'4!?N…$YµAGN4FGL J2136.2+0032?ÑV°Z7^ÀAÊdÂø7µÀ:÷Q۔çÀ<DFŸ@2΋hÔU@dZ˜Ó?ÀüÈŠrà?̙}jº@ FÇd®@ج8'¨f?æø¾&@Ü¿éòÚ/­m¿ç» !³ƒû¿ïÿùµc#¼¿î¬¢ŠÙã?ïù!bü$AGNfsrqOX 057?ïúY`œð?D~¾[Ñ?F›¹ûÎ3?D~¾[Ñ?ïë¥JQÝÃ?g[¥â
Q?dZµjÉå?g[¥â
Q?ï—ÃNÚë?ƒ¤'¢ƒ?Š>O,IEU?ƒ¤'¢ƒ?ïýȆ}C^?!Ï¿à¤?1»ÊT?!Ï¿à¤?ïüMÀŸI?DÊ3º†!Ÿ?='üSù
?DÊ3º†!Ÿ?XŸd›?•_ûŽe?Ž)âu­6?•_ûŽe?îÓ´ƒ2''?"¡(Bå?¢Ä·Ëûïå?"¡(Bå?ïò 
ne[?PLø7¨ô?Z¿êÛ½jÙ?PLø7¨ôAGN4FGL J2136.2-0642¿í¬búK53ÀC¼ƒÛÂ3À:çž?ñˆÀ<l*YoÞ@bâ'']@6¹£$]?Ä%W'"(n¿ppëGÀF@ÃÀ0²$?ïÿ*þ~ð¿é$žoí#¿âŸŠÿøÉ*¿ìCžOá¿£¿Ïg¿Asè°¿ïÿüñýAGNbcuTXS 2133-069?ïúN¥ªt?DŽ!œý.f?FÅi†È"?DŽ!œý.f?ïéïuZë?mÇtZ‡@?fŠã…S?mÇtZ‡@?ï¶ö¡²lÏ?~•V¾{™à?'BW"¼Â2?~•V¾{™à?ïúúÅáÿ˜?0\«ý
Ò?Dèð"ó?0\«ý
Ò?ïè'qö×&?i
û"U#?gm×®z?i
û"U#?ï'ÞÚ@}Ê?ŽˆY_ª¦?‹HIz/a'?ŽˆY_ª¦?ïù´PBý?"½¤Ç½FÝ?œÉw¯nU?"½¤Ç½FÝ?ï‪צè?`K>ÿÝP?mU›èJ?`K>ÿÝPAGN4FGL J2136.5+4259?Ë@æ碈xÀ:î}÷|¤À9Ê3°0´ÔÀ;´SFÎñj@RŖøƒ@Z—ÆZÂÄ?À† •÷£?š¦ÚtÖÌ?×vC=ÂXU@՞ñGU¿Öܱ±¾S¿äÁ/	ØÆÖ¿é`›š›ø¿á;4‰tˆh¿ïÿûB«÷¿ïX—;ˆBAGNbcuTXS 2134+428?ïú?§"_÷?^­·Úá†B?GbZ-?^­·Úá†B?ïó›s—?eìxž(Gè?YøÈ÷Õ·÷?eìxž(Gè?ï­DƋÑ?"j~Éh¥?"®ù•<C¦?"j~Éh¥?ïÿyÑç¶?>$Vj?ޅ&š`?>$Vj?ïúPGYõ"?HüËÔÊ?F¾ã[@ü?HüËÔÊ?ïȖMEl?Šò¬4šÊ?{´ÙWFþ4?Šò¬4šÊ?ïcæ®9'®?‹Ä˟Ç?"ƒ*8Û
J?‹Ä˟Ç?ïþ¨Gd÷?ž®ÜŸ¤
?%{ŒñýÔû?ž®ÜŸ¤
AGN4FGL J2137.4-3209?ÅOQµ2ÀGób¯È°À;0vŒNW|À<®Úb·…=@ _Nã<û´?û0"|Ñâ¶?Òy˜\؞?Ìç±"_É?ýÚu+ü@—2[%@¿ïÿß´0Õ?ïüÉ_o¿ÖC™J~(¿ÖÜL|Z¿âi[
lпíýZ~{°ûAGNbcuNVSS J213726-320755?ïûäI·¯?;tν?@o4ðm
?;tν?ïã@¾Ùf†?pºàšþ×?l¿A^ó?pºàšþ×?﹘ ·te?=,äk I?™÷Ê;ÌÚ?=,äk I?ïè™ó7?O˽0'a?gëf4L@Ö?O˽0'a?ïùàlj«?F´è¢ê·?H|á·Ï»?F´è¢ê·?ïGiÐˁk?£"Û²M-?—ÅÝø̹?£"Û²M-?ï'EŒüþ?ˆ»P\‰¥?‹nœ½PÞ?ˆ»P\‰¥?ï¬ça£‰?x.À#Èd?"Æ'—¾W?x.À#ÈdAGN4FGL J2138.3+3556¿ïå3	†€QÀ(w°ËæÀ;hájéƒÀ<}~´;@ ß³î¯u¤?ü±*ÇC ?ÎØLÈ/¯?Á>Þwšj?î3ÓÃt^@î¹[«Í?î½cm¢¿ë±K1Vº!?í˜{Ò7ñ¿ãÞ¢ýñ\ú¿×·†^ÔKÇ¿Óu3=šiAGNbcuMG3 J213809+3553?ïþuLˆ? ÷ù"ªÔ?(«;À¬cª? ÷ù"ªÔ?ïéé;©Š?ooߒËiã?fā™%?ooߒËiã?ïðM£?YYGðà¢u?_d¹?œ]?YYGðà¢u?ïàé~«¤?WRæmŽú?o#0¼?WRæmŽú?ïü[z²=??'¯i??='Ê0§ž??'¯i??ï™åhhãÞ?"¨>»5?‰†¥Ô˜ü™?"¨>»5?ïì"˜§µ?nÀ±T_¼?clñ;]Kz?nÀ±T_¼?ïºSÔFv?u°!}Ζâ?k
äÚ:—?u°!}ΖâAGN4FGL J2138.8-2055?Ó¿6™ªÀFì¿Â"OÀ;6ÍòfºÀ<ŸK·Žw'@!N¦.Ð"?øî"ã)/¤?ÐÍ>aº…?ÊÓ=ª/"ì?ü)T!ÀD(@ªL›,¿æ¯˜Ÿá²¿ä™Dàá6¿æ9¨bŠ8Ô?½)6@j£¿æâ
·'$¿©Úó+0ZfAGNbll2FGL J2139.1-20541RXS J213852.9-205354?ïùsC™‡Ñ?A<Zµù>?J2ðÂì` ?A<Zµù>?ïéõó?Zç?jØ
÷·}v?f
äao?jØ
÷·}v?ïÉXþ7©?vŠ nü2N?{S€ë­Ï?vŠ nü2N?ïñ="ù
‡?Hv(ÈÞàu?]"؁]Ðý?Hv(ÈÞàu?ïùupß*?CU‡~Ù®ç?J*;Ž³£ç?CU‡~Ù®ç?ï.Ӆ¬?'±ì|ä"?Œ9ô9ð‰?'±ì|ä"?ï¢1ÖfÔu?‡¦ø?‡sŠm*ž?‡¦ø?ïºçëó>ã?wà9ùe?Fˆ=V?wà9ùeAGN4FGL J2139.2-2214¿ïÎÁ»îûmÀG+'·þÀ:½-Œ*EÀ<f'}keª@ÎuÉ/ß@Ӛa?µø?ÀÉp·M3º¿²¢Øü0?ÙeèðïÂ@çØŽZ ?Èòdvw*¯¿ì=èîÁ¿à_$ù´Œ¿åœí ªD¿ïøÊ¿˜‡¿ïÿþ½à ¿AGNbcuPMN J2139-2213?ï×yÕj;n?qQ	v  ?tC?ãˆç?qQ	v  ?ïßžSEU?€0™²{?p°Ð.	Š?€0™²{?îýS~ñçR?'é™s
? *È£Ü?'é™s
?ïÔ[©ôۊ?]ÊN¨d¤¤?uÒ+	±Ã&?]ÊN¨d¤¤?ï>Ï2?št?žü8áÙ?št?ï€ÌŸ!?€•ü—?ÌØAgVæ?€•ü—?ïhƒ:÷<?•nç&ì+?žò‡?•nç&ì+?îï©ø{@,?Ž¶ë+`?¡`u¸HC?Ž¶ë+`AGN4FGL J2139.4-4235?ïƒ^+¯[MÀH*løQÀ7¤P«>¡À;=€Íù¦@ǘ°eŽ?þÞº))?•="½5øW?©(÷"¿P@@#L]¦¤D@Æu)LÕq?¹³V.4ñ¤¿Û:ð@ð¿àÈÎ:‹I¿Ýó§ªS¿än'?ßéà¿áyÑÕëYAGNbll3FGL J2139.4-4235MH 2136-428?ïþ­L al?%z9ÒÀžð?%+@&±?%z9ÒÀžð?ïõ*¢§?[ð:Y?Uó«'*E?[ð:Y?ïÌPʌšq?á*ŒL}R?yךı‡6?á*ŒL}R?ïÿÅRZô>ñk]ÜrËæ>ýV±Ëˆ¥u>ñk]ÜrËæ?ïÿL€®ˆ‹?ˆÒ€¦?oæWÂ?ˆÒ€¦?ïÑ.Vˆ*?†=ò:*ÚZ?whÔۇ U?†=ò:*ÚZ?ïãjÑ>ÿ?{Ë9ÍGÆ9?l•/
žøù?{Ë9ÍGÆ9?ïÿ¯¬U?­`M=? z´"?­`M=AGN4FGL J2139.9+3910?ç5büŠ»ÁÀ$$ƒDÃ~À:^íLŸÀ;íGô‹W·@ܹ©.@¦ÜG©ã?ÍþAŽë–?¥äìź?׌4á߯@‡P&3¿ËŽ²µÊQÈ¿â÷Lg·Ÿ>¿ëõTáä·¿â?°"—©Õ¿ï÷d?ð…å?ïƒ/ÊÈæŽAGNbcu3FGL J2139.5+3919B2 2138+38?ïýèÛ÷;?*Á¨rÅӀ?0¹a¢3²?*Á¨rÅӀ?ïî5è3†?k܌uÖ.=?aÊæ,j"P?k܌uÖ.=?ïÛd³;‰Ì?r­@hƀ?rM¦W<YÒ?r­@hƀ?ïû‡æîð?0%ÝΕ?Aàg™àى?0%ÝΕ?ïþäGEly?%VQÉ'?!»ˆöº!i?%VQÉ'?ï³å%ÅG®?DYú†ê?ƒ¶†Æúl?DYú†ê?ï¥$;7}_?ˆ|s²HJ?†¶ñ?ßH?ˆ|s²HJ?ïÖPw¹Ë?ikÃêzÿ?t׿2õ¤?ikÃêzÿAGN4FGL J2140.5-6731¿Ö€#¼ÈžÀDGë¿×À;&¸Lã¢À<ߺmN·ô@Z=~»œÏ@8ÇAr'?Ô2È?ïí8Go*Z@%žÀJ‹@uçâQï6?ïØB¡»&¿­}õ¤1x¿í…B>éÊ´¿ítÈ~ßY¿ïü•è41`¿ánß{ûùáAGNbcu1FGL J2140.8-6743PMN J2139-6732?ïÌQ㈷?'­4kŒ¶?yø×)˜C?'­4kŒ¶?ï·'ۄ‡?Š›KÆ3æ?'69–\H?Š›KÆ3æ?ìÒÍ"Ä6a?¤š
ú!G7?¹i–épYu?¤š
ú!G7?ïnsêÍ-?‡s4VÔ
?Ÿò16¾n?‡s4VÔ
?ïW¿.©Œ?ì÷9²Ô(?ˆª0æ?ì÷9²Ô(?î&¿'°#ý?µm¾jü{¦?­"ю$1?µm¾jü{¦?éjéò'F?³·
*SÐ2?ËÞTX5ºç?³·
*SÐ2?ç…Ë5ó×Ô?¸é‹Nœ?Ðôi"PY?¸é‹NœAGN4FGL J2141.4+2947?托Kª')À1/pyåŸ,À;»Üº€šÀ<u<;±'@u¦Vkq"@d˜Þˆ¶ó?Әíùþ?цÑ`/j§?úûs5X§@µ‡¼!ƒÞ?ëQóþ¿Úž+Cû'm¿Óä/à'S¿ç\cáPè¿á÷‹òç鉿ïÿïÕAGNbll87GB 213913.0+293303?ïúÝ@ãJ?=ó•Î³K?DŠûÇQ 9?=ó•Î³K?ïæð§÷ü?p‰™¡>??iXçè|?p‰™¡>??ïÊûSŒ´?tA~)ń?zõ'Eš4?tA~)ń?ïâa´zñc?Mþ¶-WL??mžK¯©Äì?Mþ¶-WL??ïû(š¨ã9?@qì•d²?C]•ÊóY·?@qì•d²?–ðP?–¼ð+Ž³"?‹øU³ˆ?–¼ð+Ž³"?ï‹'æEf3?‹‡ºÆ{T(?6gÇ;H?‹‡ºÆ{T(?ï‹r/?wjoöa4?<ãyü42?wjoöa4AGN4FGL J2141.7-6410¿Ô€˜_÷{;ÀE#KßÒcÀ8;"‹›˜À;ÂûB+»@Ðڌþ×@ÞbV6mz?œ5Qßµ?ºIؼKV@Z…‡"ݘ@ÇùZ"z?Üŝƒ‰¿Ýïâ+XÉ¿åwŠ~Ÿ¿äø¸BÒ¨¿éKʾՓE¿îˆŸ@¢‡AGNbcu3FGL J2141.6-6412PMN J2141-6411?ïù
	9 ?Oû6÷?K³Ì®Ž?Oû6÷?ïô†¤–Å ?dꍅðM?Vò¶…~Æ?dꍅðM?ï¿ÜÇ@ÆÅ?ç}eÐü?€Î3=êÓ?ç}eÐü?ïÿv¦-.j?6GƆÜ?+6ÜôzÐ?6GƆÜ?ïô»ã4\?Yy&ֆ?Vˆ9¥B?Yy&ֆ?ï½Ã#;ï? 	aÎÿ÷?€¬â0=? 	aÎÿ÷?ïº.2©†³?‡1TÇéŸR?tsRÞ£R?‡1TÇéŸR?ïþ`ì\'±?!¼Íò_·â?)ñ9uQ]&?!¼Íò_·âAGN4FGL J2141.8-3727?ï"öªõ?:ÀH‰GyBÀ9¢âž43À<F!*òó@9f­6Z@ÞÚ4"\?±Ë¾.ú>u?šwA] ø'?å	Ö¾IÚ@#ƒÊÐH¿Ö*¸¾«¢¿æá_¿æϋXŽ6¿édk"³Xˆ¿èt·,Q—¢¿ðAGNfsrq3FGL J2141.7-3734PKS 2138-377?ïûwÎæ
?BQV¬Ûzð?B!‡çg^¡?BQV¬Ûzð?ïë{øà?rÑô8%}>?dü"°áWF?rÑô8%}>?ïºä
3¾&?'.DÌ浛?FýdJ$?'.DÌ浛?ïüƒœŠÃF?-mx†Zƒ?;ãšàƒÁ?-mx†Zƒ?ïûleŒ]?@ó{àÐn?BNi©-!?@ó{àÐn?ïq§ø{?š]°»Å?'ËÕæª?š]°»Å?ï§Ðñl
â?‡ÿ·‰-a?†Ú®so?‡ÿ·‰-a?ïö6ïÍ?I'tEp¾?S"òŒ46U?I'tEp¾AGN4FGL J2142.1+4501¿î_7I²ÀØ×à&EåÀ;	r£‹‹À<|CécÜ@ תU(¦g?úÒéF€?Ò¸D‹ÑZ?Ѿ ™'¯?û'fŸqJ@Þ«T4¿ïר¦Ó?ïû@Ô磿åʧ=Ç
쿼Gmý´¿ãCcaÏ'ñ¿ãтÿyGjAGNbcuB3 2140+447?ïý¨¡3?(ÈO':g?2¿A6Ìù?(ÈO':g?ïåC±…Ÿ?râ4´éÛ?jû¼ÀñÀ?râ4´éÛ?ïàÍÚ¶;Þ?iäfÿûO?o2%x~Ñ ?iäfÿûO?ïâw:?Su¼<(F½?mˆí¬Å¶"?Su¼<(F½?ïýÕqÇ?0à߂<º?1TyzWKT?0à߂<º?ïn—@Š?œÈýwt¶?'-é•UH?œÈýwt¶?ïיW]²?zyˆ??t3Td´÷?zyˆ??ïƒ8-»FŠ?'A í-'?1ô"ù~?'A í-'AGN4FGL J2142.4+3659¿Óáe…ÀÉ´À(Ïå†6À:x(E™gEÀ<Rñ¹_ä@ Äbr'æ?ÿ5Hyd?À]ÚPÃè?"/Àô½å?Ê@±ád"@»ti3uM¿éçkÅ?ïýTõ$Ú«¿êí¢ò(§¿ÌžnÀ}¿Ø`ÈðŸ:¿ä2jGâAGNbcu2MASS J21422658+3659481?ïý-Ÿgf?@Àu-ò;?6"¢ÂRl?@Àu-ò;?ïð:Mè?b²¿|wŠÔ?_‹fll=?b²¿|wŠÔ?ï螨³N2?kÌ¡¾ç?gaWtEû?kÌ¡¾ç?ïø†ͺ?4ØQœX¹?LõäÒý'Ì?4ØQœX¹?ï÷¿R¿?S%Œd?Põs?(é?S%Œd?ï§û\,PÁ?"æáK	Î?†)Û¯?"æáK	Î?ïÚªž­2[?{xôÉÆ&"?rª°ÃƒÚ4?{xôÉÆ&"?ïæ6×Ç@‹?^{Xkr?iÉ(%¥w?^{XkrAGN4FGL J2142.5-2552¿±m'ŸS@ÀGý–áXuÀ:h˛teÀ<nÉìG¼W@ªü~ìC@Çùä]K?½Ùz|rí?À=
w}:@
;ƒcÍ@ãÃ"´?æ'ú㱿×Pâp£K¿çV±v/¿Ö}ê;ž¿ìÑý"ÕíÞ¿ï¥è\uKÜAGNbcu3FGL J2142.2-2546PMN J2142-2551?ïù€­ö"?B&À]ç?IýH´ßy,?B&À]ç?ïé l€?w¾wÿPç©?fù_©;(Ç?w¾wÿPç©?ïŒç$øîû?‰)i1§)ì?ŒÆ6ÁÄAI?‰)i1§)ì?ï÷ˆÂSC–?9¡*÷%
?Pî{¹­âÜ?9¡*÷%
?ïè•àH÷ã?hÿ%1	Y½?gjûÀL®?hÿ%1	Y½?ïªÿN"­?‹ÙýBþ†?…@,qÌ@Î?‹ÙýBþ†?ü‰Jc?ŽÛ`*Ì­?€ëk×?ŽÛ`*Ì­?ïì–~‡?VbSú®}?ci8MÉ?VbSú®}AGN4FGL J2142.7-0437?é}y'èûWÀCä"&þrÀ:¿)h¯À<ẕ@tÀ‡o@ö‹AèÜ?ÈÛÁœÂîÓ?§®šÑÖL?ß¡/$°¹q@ÍåûŠ¿ã:;e0ÜA¿ã¤ñ@õh¢¿åõ²Ÿ$¿á%sW±N¿æ¨ Åó?¿ðAGNfsrqPKS 2140-048?ïúA^š?@ÞÆÕ¼š?G†ú×"Ò?@ÞÆÕ¼š?ïêyÿSz?flždà¤x?e†ÚK]?flždà¤x?ïå
=€>)?jÎٞï¨E?jò€G?jÎٞï¨E?ïòšŽƒˆX?ACC	ý	½?ZÊãVd°@?ACC	ý	½?ïñƒV….?Yê:sQÜñ?\ùØø?ôb?Yê:sQÜñ?ïŒë Íj?Œa
$ÿ»M?ŒÅÐûœ?Œa
$ÿ»M?ïÉ"ïû?¾håØpŸ?{@{ÇÖÖ¬?¾håØpŸ?ï¼5b¸[ý?p•H\~E×?€ò§Eâ^ñ?p•H\~E×AGN4FGL J2142.8+1958¿¯‡3p²ÕÀ8c`9%»{À;°)(vÀ<ŠxËøQ@!q¹7C¹?ù_=?%°?х™ž!?ÈA÷[ÁœÃ?ù®} ½ê@	XfŽTl?渘B+ž"¿ì%ôïo¿ÄÝ·*Ï¿ÍØçø¢=­¿â?`A^D¿Ê4³{mÂAGNbcu3FGL J2142.7+1957NVSS J214247+195810?ïÿÅ¢ó?Û{ãñI?GPÄ ¸i?Û{ãñI?ïè¾þØä?mêpWÚt?gëA'¢¼D?mêpWÚt?ïñ*³"ü?OÞe+uö?]ª™Ê؈?OÞe+uö?ïùí|o½'?1}¬èçÚ?HJ
šwí‹?1}¬èçÚ?ïÿd ÄÇ?-?ä<sw?n"Œ'B_?-?ä<sw?ï'	¡y"?'øÃÈ,¯*?‹½º^€Öå?'øÃÈ,¯*?ïêHx"¼:?op}¼Sæ?e·‡nuÏ?op}¼Sæ?ïòa©¾)ò?L4¥ŸVò?[<¬3õ,í?L4¥ŸVòAGN4FGL J2143.0-5501?ã0û»LǯÀGh3Æ*À:·"òsOƒÀ<lꭈcç@jŠbo@…ËÀ]?Õ¦"»ë?ïÿšr¦ç@Ĉ'ðà¨@gIh~¿³Åüà!#¢¿æ¦²¡¨[Ô¿ïþdõM—?ïp¥ïé1‡¿ïÿìIiÖ]?ïŽéõÒAGNbcuCTS 0561?íÍÐwlH?¾"ôµ¸ÍÖ?±''ŒÏÁ?¾"ôµ¸ÍÖ?ï  †^1?›ƒƒMiú¡?‡×ül&ã§?›ƒƒMiú¡?íyŽEê½?¡Œý"jۖ?´3}b¶–?¡Œý"jۖ?ïÅÐËVT?vʒ\à=?}šUH2Q?vʒ\à=?ï˜9
žÐ¡?ŸäÜî?ÿ˜?‰ñ½Jg¾?ŸäÜî?ÿ˜?ëÙÕla/Î?É®a¬G‡?À˜ªN{@Ç?É®a¬G‡?ì¹Ö´?ªæf‡
°9?¿:1Oê_@?ªæf‡
°9?ë' Êó%I? ž'õ ?Ãc|Ô3jÞ? ž'õ 	AGN4FGL J2143.1-3929¿ïH}'róÀH¢ÛߏG0À9õƒ.I½À<W"4$Ê»@´çër@(¯œ:]Ê?´F¾?ì)4¿xÁ—©CJ?Ÿ±m@ôÙjM?ë.Áÿ"JO¿ÛWUý7£°¿åJàc'†X¿á'K3Úøß¿æ!ú[{PÙ¿ÌËc@A8¯AGNbll3FGL J2143.1-3928PMN J2143-3929?ïýº_þî?="ïü,?2/m©[³ê?="ïü,?ïì'È-Åz?krO÷²?cn7áXÎ
?krO÷²?ïÓÆ›5â?|§¨èü_5?vüË">Í?|§¨èü_5?ïþZ̲Ô1?@£³´7?*S7G¼Ù?@£³´7?ïü{¼—~?Ckzý÷ïÇ?<"½Ÿ?Ckzý÷ïÇ?ïl
ÕU²d?›ÛÇ*eH?'~ENj{‡?›ÛÇ*eH?ïÈVs)Bo?"cb,õF^?{ÔÆT±\Ø?"cb,õF^?ïýWˆõS÷?)NºsŠ?5C¸Å†»?)NºsŠAGN4FGL J2143.5+1743¿ï«"õ´¼OÀ:غ@ÙÀ7gþR€ÖTÀ;iÍ9VÍ@ù§>Ê@šz…\!?5…¦{2?£gQ×kâ@
…bÅÇõÍ@^'Š]'¿Ñ±U¢ô·"¿äâaÿÏY¿çRºýÂc¿åÉVAU¿è}ÿºà¼¿èÌ{n5gÁAGNfsrq3FGL J2143.5+1744OX 169?ïýê8dí¸?$­Œ`Ù?0®=×.?$­Œ`Ù?ïçõÓ	?qÐ
§èý?hæ
hC?qÐ
§èý?*
è?‹$MtúiB?ˆ?ß'¾?‹$MtúiB?ïû6´
øÆ?:2ֈÁn¢?C%/;Ԟ??:2ֈÁn¢?ïü±h10"?8‰ÝöI?:t¼ýYzB?8‰ÝöI?ïy¹•kT?š>I²h¬ï?ÈÍK¾=•?š>I²h¬ï?ï–é°!4G?ÏɊFA?ŠE"Â5?ÏɊFA?ïón~&»D?]Œ$÷hOG?Y#üÁ?]Œ$÷hOGAGN4FGL J2143.9+3337¿æ_–éfÀ-s¡ƒrçÀ:ÆXaÀå8À<iï¤h)µ@ aê»PR?ÿÑ*)Ÿ6?ÃZ°ûŠûF?«*n­+È?êpå^"
?ý¬ó@T¿ïù¥þÐ¥?ïÿû˜'2¿¤ÉlßÁ
¿ä²¥~Õ(¿áy‹X࿼ÚÝܔ•úAGNbcuMG3 J214351+3337?ïýHzý?2ÿôó֖?5¼+¿
Ú¤?2ÿôó֖?ïáªX±?sN«ì¥Ø´?nUý oÅ·?sN«ì¥Ø´?ï¹ÒÍJ~²?"€ÐП#?‹L£"?"€ÐП#?ïÈŘ>êe?a(ZŠœ?{3õØa9?a(ZŠœ?ï÷ŠåeŽ¿?M<÷‡?Pê4¹0'ä?M<÷‡?ïXõ
¢nÄ?¢ÀIܗðø?"á^K²'|?¢ÀIܗðø?ï¼=Æ4,W?‡¢6õUD:?€ðŽjî/?‡¢6õUD:?ïõÿÊ?‹x7ËӐ|?ž!]ÅCp·?‹x7ËӐ|AGN4FGL J2144.2+3132?ãjºŽå>;À0M>Õ'å!À9§<t$•À<+ºõ3ô#@S0 U @ƒ¼ûžqp?³êoJ×?­Y2Ý^%¶?ø"c¯ÒÁ@
<'A¹2ç?ïË}ÂM—ã¿ßAݨ[S¿àá–5df¿ãªŠLõ|¿Ùʊ<ÚPï¿ê) ¡`7AGNbll3FGL J2144.2+3132MG3 J214415+3132?ïþÄ3ž? ‡_H¯`?/³ºùÀyS? ‡_H¯`?ïî?Äø(V?eüe*
	?aÀ:ûy ?eüe*
	?ïòXAWÁ?a¢úëìì3?[O}ˆð=»?a¢úëìì3?ïñXzjP?C¾ˆÄ•/?]O
È¡?C¾ˆÄ•/?ïû&òˆE?9S`?Cd6ï«ù?9S`?ãÞó?šôaÄɦ°?Œ"ûùIÓ??šôaÄɦ°?ïêÝØe?qïy_pÃ?e"ä"€:Ô?qïy_pÃ?ïÙ°4ˆX?_àXñaðI?s'å£8£è?_àXñaðIAGN4FGL J2144.3-7802?ê9†^m7ÀAuäõ8&À:l&ûíLÀ<£u»n@ôí}F}@C…%nN'?ÓÀ£~tÐ?ÐM`…ü¯?ödŽTÁù4@
3Ï.Pö=¿äþ÷Väd¿åv…}'âž¿ì"+
oÆ¿ïüë"£C?ïÂ}h‹…¿ïŝù¥žAGNfsrqPKS 2141-781?ïý¶•4…?6º"ïaï?2O¥®o?6º"ïaï?ïö ŠÒ?ZM"" Có?R¾ì-rüb?ZM"" Có?ïMEfB$?'CÅç/™?–WS7°Q‰?'CÅç/™?ïÿôLÌ>ØneÐ_Ö>×fdåjH>ØneÐ_Ö?ïý¡¬k6
?>3ÌHVGæ?2òhì­Õ?>3ÌHVGæ?ïÛ~ûL€Ñ?s¢FÔN2?r@'G1³§?s¢FÔN2?î©°´NŒç?›ÉŸJýb?¥dôº;J?›ÉŸJýb?ïÿ
œ¼
ã?$_"‡ '?¬nóî9?$_"‡ 'AGN4FGL J2144.8-1817¿ï¢Ð£WCÅÀG)ayWÀ;h¥IÑjÀ<ºqÊG·O@ ä²hG'?ÿaueݪ?Ì r}ËÞ?uH¥qzQç?¼ßŸb±P@vO[‡æ¿ïýQßñ—²?ïÿÔÌuŽø¿â
Ò¡"$¿æ¢f&¥†7¿µtSäوó¿â¿ý¡UûŠAGNbcuNVSS J214442-181801?ïýö3ùW?nA7Œk®?7ØL±3?nA7Œk®?ïî¾ú‹?dœSиó?aAà
ôP!?dœSиó?ï×["qï?v®Á€\Á€?tR6iÚ [?v®Á€\Á€?ïý›ʧ.?"쐉‹3ç?3';›ÁC"?"쐉‹3ç?ïýûн¿‹?,—pŠaŒ"?0!zÏt/?,—pŠaŒ"?ïO¦%?'Êá¦}̗?ˆº¬ÚÖ?'Êá¦}̗?ï½®'£V?''K§ÑÉ??€"[…ürœ?''K§ÑÉ??ïôÙÀ?¢?Páz?VL#?PázAGN4FGL J2145.0-3356?ÜÝNTºÀHÐGG"#À9HÆBoÀ<÷ïF4@֒­Â—@O,e¹˜=?©-ÝÞÂî}?¾&•Q¶@³w[0@»Õ]jo¿»v|3,RC¿Û–H¬A<
¿ãø#B$g¾¿æhH‰͟¿èÍÃØ1"Ý¿æ]THÏAGNfsrq3FGL J2144.9-3356PMN J2145-3357?ï÷wx\ˆ?T÷eòŒÉ?Qj«Ã[?T÷eòŒÉ?ïä\çÈ·Ð?wôç±?k£Kï¶?wôç±?3[!?ˆ›Ö£˜Õ?‰ûÞÀ租?ˆ›Ö£˜Õ?ïþ+N¸IÞ?µ%#Ô0?-Kî¥Tþ?µ%#Ô0?ïê•ZÎ5`?iâ…#s€3?ej¤ü0¸?iâ…#s€3?ïZo×B5s?¨Q¼ýu+é?"²Úœ?¨Q¼ýu+é?ïw±àÇù?V¢özö?'	ßãçç?V¢özö?ïûXQ"?7¶ésú?Bž»ü†d¡?7¶ésúAGN4FGL J2145.5+1006¿ïïÚ²#åIÀ?ŒÌxéö©À;^.†%HÀ<§Î_ª@!í9Y=?ûY'ÿ?А›ëÙ?·Š¼+R?êϔÈy€õ@.-%Òø`¿ïÿÆߢèM?ïì~Bûþ¿Úd\åX¿ÚÇýsޟ¿Í–ÿöÅě¿ßôâ?¥²AGNbll3FGL J2145.5+100787GB 214302.1+095227?ïÿ«iOÏÌ>øþUù^Õ?%¸ÑŽü8>øþUù^Õ?ïê§Ó'¼?jüñÒ?eX,k]¼?jüñÒ?ïõá™«à?T˜zñÉí†?T<ÎT›¿?T˜zñÉí†?ïýÑó¹?·)Åþ†ž?1wöQ8Δ?·)Åþ†ž?ïÿ¨`ÿÂ?û_?''?çÂÇ;!(?û_?''?F؛Q?•˜CÚՋÿ?Ž.?ŠWÓ?•˜CÚՋÿ?ï÷C‰JI®?[
[¾?Qxíc-"h?[
[¾?ïøž8~n?F	çšøË?M‡Y+	?F	çšøËAGN4FGL J2145.7+0718?èGӍJÃÀ@´Â	$lÀ:µmÖPÚÀ<]¸"Üû@ q›#òÎ@Ñ|^?Åçþ×`ú¿•vFáÄ^G?ÒoÞ_FaŽ?òH›—ËŽ3?ææ¼Aå'·¿ç^-¢¥†ã¿é_ωþœ¿Ñéy«½ˆŒ¿Üœ\AŸ\§¿ãh4ë~AGNbll3FGL J2145.7+0717MS 2143.4+0704?ïø‰#TÃÒ?S3ÜòN?MÛrŠNC0?S3ÜòN?ﺤšß?Œ½
ž$ÔÝ?~—ÿÂ?Œ½
ž$ÔÝ?ïÑބ…5_?yñãG»"?w½Òø ?yñãG»"?ï«+<ø6'?h)óÀí˔?…50·£‡é?h)óÀí˔?ïßlÇ©w]?rüû=vv¶?pIœ=Ò5O?rüû=vv¶?îŒ\¯$è?¬WͼùÕ?§:5Ր?¬WͼùÕ?ïÁѽ]ª;?…Ê(¯VZ?!^9f<?…Ê(¯VZ?í´`Ÿ§û‡?›
á¿øþÚ?²\ûUÉ?›
á¿øþÚAGN4FGL J2146.4-1528?è·	'¼fÀFÑ|¯Ý©À:YyîÙgÀ<1£üÉêš@4I'n|à@Ì·ƒl?¿Î-_‰¨`?¿­0û›|?ø¥Èçdþ‡@ëɃl0«?ïó!3F¿ä½U¡E¿ëa¢ýpƒ¡¿é¡YìÛ`¿ëõ ޜØé¿ïÔ+{¯AGNfsrq3FGL J2146.7-1527PKS 2143-156?ïûúö÷?9šÄÈ{°?@(Û^?9šÄÈ{°?ïìÑGŽg•?h¶I­­±?c.¸S[Û=?h¶I­­±?ïÀeÔ×C"?|ö<÷J?ÍŠ¿UÓ?|ö<÷J?ïñÂÀYvê?F.¹™(i?\zŸˆÌ?F.¹™(i?ïⷓ»ÅO?wó¿pfò?mHl+}h?wó¿pfò?i:ðÜ?‹E
/µ£†?‡ß¥±CÉ?‹E
/µ£†?ï#ö¥õXÃ?—¸²Ÿä‡?›+Dă'?—¸²Ÿä‡?!úQj?nÅ)ñ
D?€ß˜~«õn?nÅ)ñ
DAGN4FGL J2146.5-1344¿ï}†µU%»ÀFy—Ý÷wÀ8ë¼3øUÀ;‹Ûϟ$@Όïg+ˆ?÷ëŒ
dÝÐ?°y½!3+?Á±³ì{i@)4ÀÑìÇ@fûc
@…?ïGM1:Ç¿Ô[â¿Ó·'I%¿Ì¼&'j¿Ù"­‰'¿áœõ~DZ/AGNbll3FGL J2146.6-1344NVSS J214637-134359?î>J'ÚĘ?Ì«¾pyËÚ?¬VâS¶z?Ì«¾pyËÚ?ﴓ•žI?"§Õ:'I¯?'Û"=%±?"§Õ:'I¯?ïpËß^l>?"æßÈ}?'æ"°*?"æßÈ}?ï´c²ú5?kê6¢Ðæ<?'üçÙ¸·?kê6¢Ðæ<?ï  ·££f?–LC†"Â\?‡×ÒÈRy?–LC†"Â\?î±Ã1¥?»hdåª?®´ãÐ^!ª?»hdåª?ÖD?Õ
é%
¥?>8H;›?Õ
é%
¥?îØ¡ñp´ã?'à"Ã&cu?¢uàæ`üØ?'à"Ã&cuAGN4FGL J2146.8+0425¿ÏM"%™öÀAµB€®IÀ:—Ù
LïÀ<3ycՒ@ò¤ø`@E"FK=ì?ÈèÁà_¦¯?Â4õ«?ò¸M¹Ç7@¶Å4ý㛿萘~'€p¿}è(a·Ä¿ê@õ~丿ëd&ñ'9¿Ç=Xlþ†¿ïÿÿÊPËAGNbcuMG1 J214653+0427?ïýğ_^é?<ύó·ó‹?1ÛÕÁM?<ύó·ó‹?ïêa£'ª?j#
›¨ù?ež\‹?
…?j#
›¨ù?ï"N¾vj7?‰o{`]3?‹,PT§U?‰o{`]3?ïýŽ*û@?" YŽ?3Ž§_%ù?" YŽ?ïÛn'Ò!˜?'0<«¾s?rH¶wRÌF?'0<«¾s?aúœ?"Ò`¼V¨›?ŠÑÿÖSM?"Ò`¼V¨›?îÐ<®\d?=a³™âú?¢ü5>Á?=a³™âú?ïé¼'¦í?^ä†îïPù?fCà) ã:?^ä†îïPùAGN4FGL J2147.1+0931¿ï1LÂëÀ@×ÆûÒtÀ8h5qÑÔtÀ;Ò!¯}0­@'š¤†ˆ@u…zþ£ß?¡÷Hõ™L?¹"ö%j@t¥ß"9ç@h[J©q~¿Ï"ϝŒ˜T¿ãSßà›¿ç·|¯Ý©¿èØÍ÷o7Æ¿éd=ÔÌË¿èÈgÕÒ/AGNFSRQ3FGL J2147.2+0929PKS 2144+092?ïün-¸¨†?2
¿2 p?<Ž"ò‰Ì|?2
¿2 p?ïàÆÈ/?' Œ]g"?oýáyÐy?' Œ]g"?ïÏ^ޙ ?y:z¡)I?xPÿ¡á;Å?y:z¡)I?ïþâónñ?vñjϒ'?!Ð˃х?vñjϒ'?ïüãÐkà?0HÃ&8D?8á~»1Â?0HÃ&8D?ïkY†wö?œƒRP£?'"Þ*	—B?œƒRP£?ïÞâ0"?y£Á†Å?pŽøáÀa?y£Á†Å?ïý4RÞt?+3x{øÉl?6_
Îó?+3x{øÉlAGN4FGL J2147.3-7536¿²,õ®!ÎÍÀBDR½<6À7™I¬|À;Œ›aöK@ÅeÑÄ®@íüºÑ!Æ?"~<*©?±>uf3'@;8 ؽœ@²\L=Ý¿¹¦'ác^¿ã‡>ùºì¿æ18‡0
Š¿æM= t¿ê‹P*º¿¿éWòeÊAGNFSRQ3FGL J2147.3-7536PKS 2142-75?ïøO'RÑ?Qwˆ¥¾ž?NÁ÷Á‡£Ï?Qwˆ¥¾ž?ïô&!Ê!™?f$>Ùúq?W³¼^E?f$>Ùúq?ïÉtÂìñ}?}Øg
'W§?{Ežvù]±?}Øg
'W§?ïÿ͗;à>òsd|ǚ>ù4yáf¼G>òsd|ǚ?ïøüäu=¢?Bg5""9?LnïL¿3?Bg5""9?ïюv™@?~kґ}Ûi?w8Å¡ß?~kґ}Ûi?ïÑÍ<´;[?€Ì"•9<×?wa°á6?€Ì"•9<×?ïÿŽI? :?	Ë>Ÿ
Ø~?m¼]èYA?	Ë>Ÿ
Ø~AGN4FGL J2148.0-0733¿ËãÛq5ÀE6€àe0À:S¡"I¦<À<j|>>ÿð@¤—»H?ý_ÂÞ6œ?Ä	Æ'l*¡?»JµA&!8?õ¶{ò¿¥@5˜þ")?ítM_.cÁ¿é§ ÉN=¿Ó +ïrC¿ÖH´å$‡t¿äú¬¤8Y
¿äÌqæÍAGNbllSDSS J214807.08-073347.0?ïû_á€Ò½?6Ĺ!]ˆ?B€zÄDÀû?6Ĺ!]ˆ?ïåì`äi?qêýê
›?jŸO.à?qêýê
›?ïñdèU?^Æ}ƒˆ"?]6ü`Ï%Õ?^Æ}ƒˆ"?ïÕp:á¹?Z1—RÇ??uG⋸t?Z1—RÇ??ïóöŽVd?N}ºš"?X㘧gt?N}ºš"?[X…?'Bá4lª?Ž))Þºz?'Bá4lª?ïë7ðBƒï?tbœB?dȬýðÍ?tbœB?ïòí{v¡?v¢"9'XÂ?ŒƒD–Óƒ°?v¢"9'XÂAGN4FGL J2148.6+0652?äûc¯ì†ÀA™í|o½À9ñxKk8]À;ô÷Zï:@Q·&tU@BªA‡‰Í?²•>9x?ÎÃ핚0˜@jgÀ¹ï@
`ç\ðñÅ¿Ê-ªÞ•I¿åÖ]9–úƒ¿èºk5Øÿá¿ëƒï¾"OÙ¿ïÿúŒ—Ó?ÛÂð?˜œDAGNfsrq2FGL J2148.2+0659PKS 2145+06?ïí¤"jnš?†[,í'?b[{¬î½è?†[,í'?ïáŽjo?"÷ÓÒÆD?néqt"­ô?"÷ÓÒÆD?ïžT?ûÌ?	•ßዦ?ˆ}êðù?	•ßዦ?ïí3SX[{?Lºµ.³º2?b̬©]j?Lºµ.³º2?ïí"I?'ø?jÐáòeú?b{¶…¾Àx?jÐáòeú?ïNÎo¹+?š®	UMÁ'?–&2v"?š®	UMÁ'?îµÊf.÷Ô?–ˆ;²º{1?¤£YžÈP¾?–ˆ;²º{1?ï4þhvÀ?ˆ¯É¦fõ?™`>oŒ?ˆ¯É¦fõAGN4FGL J2148.9-0121?áVÙƘÀC£2œ4~À;Ïëe>HÀ<YLÓi©@Z$×$êp@ºñ-À?Àî^—ååM¿µ"ÄÐÿâN?öÃBZ£‹?úäd¬R?îŽñ"%¿äCHT,§ÿ¿ìlü›Ç¿Ü¨¡õ2Ç¿Ö5²~íÆ¿°Bœ ¡O	AGNbcuPKS 2146-01?ïùà+º?H&ú‹'§?K°}dªƒ?H&ú‹'§?ï¾îöså?
¥eÖ?€DBoÔ2Ï?
¥eÖ?ïÒNtŠÉü?xD²_ÙÇl?vØżªÆ3?xD²_ÙÇl?ïê"IÀQ?T£p¾¶Ÿ?e{¶p6–?T£p¾¶Ÿ?ï͇xÀí,?i'!Û#?y<C¡™.?i'!Û#?í²ãq?¹&uÉPƒ‹?²oûø×ù?¹&uÉPƒ‹?ï–íD'o?‹Ô-eÕ!#?ŠD®Ø0ˆR?‹Ô-eÕ!#?îÀijE3³?›/$ÒÓ¤?£ó´Ìˆ«Ì?›/$ÒÓ¤AGN4FGL J2149.1+6104¿ßÑ׫–!@mœBÁE°À9®cÂG7ÍÀ;{Š '§@©ù
G'@W¬Óª7?ávŽöS?Û	tBÈ@ò³Ù¶À@	ٗ
ô¿ÔÍÂ6Ƽ¿æÛz_A®÷¿ëáûbó¿ê(úãe¿ïb>ï)'¿ïŠ‹>‰AGNbcu4C +60.32?ï¹wõé?¼Z[&}~?žÐýì¦ó?¼Z[&}~?푂û-Äp?¶úüP)*t?³sè&#é?¶úüP)*t?íO¸ê9;­?¢§)Y}H?µ'8¬~T˜?¢§)Y}H?íѪN¯?""À+7?±r¯|EP
?""À+7?îM€OVæ}?¶å§Z¿—š?«'ûÙÊ5?¶å§Z¿—š?à*\O?Ô)»`?ß«Á×GÇa?Ô)»`?êôº°G?­Ù4Y
ù§?Ǽ-?Šã?­Ù4Y
ù§?Õoˆ&é,?¹îŠLI¯¡?åH;üì‹j?¹îŠLI¯¡MIXED4FGL J2149.6+0323¿äÙ:;¡RÀBNpCßÀ9Üëô°@¥À<F։äð°@ú‰*`¦´@êOyº×?¸N\Yr7*?«yQ'æ?ñS(ýOL@$xy8{¿¸tGz'î/¿çOš¿à±Šâ¾w¿áX¾]g¿èöTOãm"¿Ó[Þb¡_âAGNbll3FGL J2149.7+0323PKS B2147+031?ïüÃ%¸?7-ÐxçU??7·ñq«Ý?7-ÐxçU?ïì,šmÞ?jjù x܏?cÓäN4ʚ?jjù x܏?ïêÍ!ls?de#úÛB?e2Þj'<å?de#úÛB?ïüùý‡?*ÿŒÎWœO??/næ9EÌ?*ÿŒÎWœO?ïðÇÊÇÉ?Z½)Ó¦?^pl&'\¿?Z½)Ó¦?ïšfuLTº?S>ÙiG?‰fb·9¥"?S>ÙiG?ïÒsg?~GtžUË?vÆyåáÔ?~GtžUË?ï÷6nsa?A6Îò?Q"Þ÷=ƒ?A6ÎòAGN4FGL J2149.7+1917?ã͕óØærÀ:ZS2­À9ë—i=±;À<ó"Çz@4K¯«Ô°@·Zï9ß?½À©}è88?·Ù\Á殏?õ°
fóT@%÷5¿ç•žˈ¿ÜX'¿Ä¿çOÁ´?ã¿éxM·‡¿ãĀ˜@Ô¿ïþž
ÇAGNbcu3FGL J2149.6+1915TXS 2147+191?ïý㪬2ñ?TK–\»?0â©f%•w?TK–\»?ïî¯õóÙù?eܦ[4^J?aP	ë)ÆÛ?eܦ[4^J?ïèžÄž!‹?l—c.¬?ga;åõO?l—c.¬?ïþ€=tw?e3˜°²?'ü+²((?e3˜°²?ïþNìïyl?'è
 )ò?+,øEä¼?'è
 )ò?ïœÉä(ø¶?'¨vÓ²I]?ˆÍ‡€BO?'¨vÓ²I]?ïÄ{2r»?€ÖÏL>	?}ñBs%:D?€ÖÏL>	?ïúnՏ'Ù?9v¾
zð?FDª9@¤V?9v¾
zðAGN4FGL J2150.1-1410¿ïWôÕ÷»ÀFö5"_õÀ:¦‡¾¥ÃÀ<1£Œa¢²@ ×ÅiV?ù»À6âë?Áb@|që€?Â2‹˜z	Ü@€	ö#l@ՑíRÔ?îyˆLj;Þ¿çká©Ó¤¿µWXvb¿»^¾Š¥ò¿ãïî:ތ¿Ôéâéj'AGNbll3FGL J2150.2-1411TXS 2147-144?ïûÊüò?8	'ò­H¸?@ׯ?ȋû?8	'ò­H¸?ïèzzšzë?lXzKĦ?g……wcä?lXzKĦ?ïëlÑuº(?e'•®ê%?d".PŒh»?e'•®ê%?ïÁ­ì¯7³?bïêyÎ?)	™Eޟ?bïêyÎ?ïà´Òr>?j·™	L?oK-ük¹ ?j·™	L?ï‡Úûj?"¹B@I?Ž9‰K‰9|?"¹B@I?8D{@?ŽãÕm~_a?Œ–²;Õ?ŽãÕm~_a?ï_wL›AÃ?Ú$

å?"q¿1š?Ú$

åAGN4FGL J2150.7-1750¿ÖaŽaz½ÀG¼Û¾WïÀ:R}ü…!=À<ZS¸ä¸|@<pšœÎØ@2M	žs?¿Ã±ðþZc?ŸªžÆ÷m,?àv©ò´h@·FRʨ?ïî6>€nO¿ç8å#Û§[¿ç§¿Í
	n¿åà½D™¿äÍcˁs2¿ïÿÛb;ßTAGNbll3FGL J2150.5-1754MRSS 600-040574?ïúè]ÄMÅ??Š0MS˜?D^‰ËÉeÍ??Š0MS˜?ïëz¹üÝÙ?mµ}CƒR§?d…F1ÜÖ¹?mµ}CƒR§?ïä!×ãx­?cò}²œ˜§?kÞ($ÆbÂ?cò}²œ˜§?ïí4.csK?MhûØHâ?bËѝì{?MhûØHâ?ïöÄÿ'¶•?O~W¦?RvPÅdÙ?O~W¦?ï–4þ^P?'H0—ã¼?ŠrøG£×?'H0—ã¼?ï®éÅV
ú?'ÐKqræ?"EŽ›µ?'ÐKqræ?ï§\BÑ?s{3›™"2?†(þ¬ïÊ?s{3›™"2AGN4FGL J2150.7-2810¿Å±ƒ Â~{ÀIâ`²È?À;^Ý÷—À<",·/¢@ 6üªàéº@%…EN¾ª?Ñrª?ÄÏi_?*¸?ôKà©"£™@ì&ØÜÐ{¿ïþÁ?|?ïþtå…*w¿ãàH	"
@¿Þ¯°ýcmŽ¿áøžö{¿àÖv~â^/AGNfsrqPMN J2150-2812?ïþyP+š?$Í÷b?(k‰Ð?$Í÷b?ïîq?æÓg?càp˜ñ_s?aŽ¿ÛS¡ˆ?càp˜ñ_s?ï×帽1Š?yŽ£‰…}?t
#½"?yŽ£‰…}?ïúJÊ®Ô?4÷™1ë†Ù?F×솧9R?4÷™1ë†Ù?ïýû0Àð©?1`zÈá¡?0&xS]Ì7?1`zÈá¡?ïš´e‰?'w#þX?‰~í|÷v?'w#þX?ï¸üLl??"Q'Q–r?üîô´,?"Q'Q–r?ïÞöÍ?iIùçkÃ?p÷ôÓqm?iIùçkÃAGN4FGL J2150.8+1118?àõS2úJ¬À?»5*"8	À:å!ÁçãÀ<2\sž]@¸ˆd@H{Ã?ÎÁ".öŽ?¦cžœ?Õ=îãx	ý@ý]žk»e?íÜêâ6–j¿êåídòÈà¿ÙziÓe¿ßÀâ³¾Þοä´Ó˜A¿Ñ–éÜ'2ÊAGNbllNVSS J215051+111915?ïþY~ÃÌÀ?!'¤Y±??*hÛ ?!'¤Y±??ï秆8¶!?rž·ÙÕ,Å?hXy¤íÆÔ?rž·ÙÕ,Å?ïør
þ4=?>—_CÔ=?N7ÇRPjê?>—_CÔ=?ïõÞÃ34Ð?5©5viӈ?TByäq£?5©5viӈ?ïþ¹ƒfH×?Uv—ÿGö?$gÍÁ"i)?Uv—ÿGö?0VVp?'=)¬ Û?‹SóæúÇó?'=)¬ Û?ïö(êk)€?f",)¦?S®*×6`¤?f",)¦?ïàˆP›ùÆ?Vþ#zç#|?ow¯t"Y¿?Vþ#zç#|AGN4FGL J2151.4+4156¿í•ÏrkéÀ"͒·þ¯À:_úŒ"¸'À<Ib(D€@ [ÿûù5?ù´ýö°Ì?ƙähŸÒ?ÕNŠø.%@«dÅ|vs@ø~©©1<¿é@¸Azsº¿æx6ÝâžÆ¿¸ÆÚVM?¿ÐäK3''¿áñBwô®¿è>ôÈAGNbll3FGL J2151.6+4154NVSS J215122+415632?𢡊u~\Q?ëqÎZˆ»?…"§H#?ëqÎZˆ»?ïÆIË{?ƒÍ2Ê÷9?|ÛF•ú?ƒÍ2Ê÷9?í‰#ŸíE¾?¤²þ™?³¶âþp'?¤²þ™?ﻝˆøÇ?cjMΫ?±xJ?cjMΫ?ïWÞ¨\?¼ûû6ã.?œ•.nð|?¼ûû6ã.?îäû/"JÙ?¬h>Í?¡°M—9r?¬h>Í?ëúîox¢˜?®Þ_ûƒƒ?ÀFBu¡?®Þ_ûƒƒ?î¦
¨µv?'t"Ô¥»?¥Ÿ%xú+™?'t"Ô¥»AGN4FGL J2151.7-2749¿æ»à'óÀI-ž×ÆûÒÀ:ªDkiÛfÀ<0®û*®)@Ó/Â"'@[*'ñ¶'?ÖómàÙ??á4±¸tP@$è'4ù@
f´¯Êˆz¿àÃNžÉ"C¿å–Û¿
¡¿è¬R¾éµ;¿ê¢"FY¿ïÿþøþ"?ïòª¬çT8AGNfsrq3FGL J2151.6-2744PMN J2151-2742?ï½ßÕEÊÃ?³ v³‰±y?€ˆ
ªmÇB?³ v³‰±y?ïç½»¯:?{xûjÍ/?hBD:Çó
?{xûjÍ/?îneÊpbO?œNôz}Ùü?©£[?œNôz}Ùü?ïõìÚoˆà?B¯!NÁ'?T&JÖ¶°)?B¯!NÁ'?ï÷qFqÜð?a'pŒGà?Qs"º?ÿ?a'pŒGà?ï"̉l6?'í(þJ?ŽÌݯAM]?'í(þJ?ÒÄ*? nV¢]"Y?§ÅbÖQw? nV¢]"Y?ïºá7	xò?vÒ«Cõ'&?G²K`3n?vÒ«Cõ'&AGN4FGL J2151.8-3027¿Èý(":ÀIb@îÙÀ89ÔñhŽÀ;¿?úÁҞ@æ°d@ýÙ<FØ,?¢T=nöWá?Ç°|ʀí%@è_^4h½@{Ã;~†C¿Ó¡ZX;*x¿æ‹a]¿ë¡}¾œ³¿ìàYq‹^¿íS›R×=i¿ïéjÇôö¸AGNfsrq3FGL J2151.8-3025PKS 2149-306?ïV|Îݞ+?µÓ4M–_?•0f ܞ›?µÓ4M–_?ï×D͏jl?"Åùñ^µ?t]™>z ?"Åùñ^µ?íŸA¥M>?¤£}3Œ"Z?³òÖa'?¤£}3Œ"Z?ïú@""å-?;(îvø?Fÿu£A?;(îvø?ïf¬ÄªÑ?•‹à¨´°?"0
l'è?•‹à¨´°?ï07Œ¢ÿä?°%?Ð["Õ?™ùh0g'?°%?Ð["Õ?í3Á¸òz[?¨"´'Œ?¶aò8l-%?¨"´'Œ?ï×*g,µ?j5·ç?tjû¿[!?j5·çAGN4FGL J2152.0-1205?퐰84ÀF¹‰›õ"lÀ:Îÿ€¾À<k¹›— ›@ #Ýqµ¤è?þ%鞔«?Ñÿm]ü_?Ë!]•Ç?ýíG+7¼/?ÿ"IŽ¿ïýPÒ8r?ïÕ}«&‰Ø¿àÛá¨&$W¿Ûf®_ÏH}¿áP«>¡%¿ïÿä¡Õ¨>AGNbllRBS 1791?ïòËPÃ3h?Vt_M±Ñ?Zi^f[_g?Vt_M±Ñ?ï¨Ñ´#nÖ?–Gâd0"ª?…Ë'÷$Js?–Gâd0"ª?ï°·~Š
?}'êÄsPÉ?ƒÒ8pۜ‹?}'êÄsPÉ?ï!aŠÅ§?paßã'Ê—?Œ7§«
?paßã'Ê—?ïßYdÓÇÆ?kÛ
÷tI3?pSM–Ò?kÛ
÷tI3?î
ýŸ1g?ºÜ$nk¦?¯ ."U—?ºÜ$nk¦?ï4?£ÀQ?"Øüݖ¬?™x‡üî?"Øüݖ¬?í~õPF
ô?¢/û¶¾DS?´U}Ϩc?¢/û¶¾DSAGN4FGL J2152.5+1737¿ÀçHŠ®À;°¸{Üð0À;óiï‡ãÀ<aŒ¤¾Ê@zo÷ß @å^¼Mùˆ?͇4|´['?¢tâCñ5Q?ҝO0¿»l@ŠšrÝm.?é'Nž·Ì¿âZi7Ñþe¿æ]¾Anµ?¿ä$à¿ÈØL¿ãÎAvÂÔü¿îô›GðAGNbll3FGL J2152.4+1735S3 2150+17?ïþ~±ÇôÝ?"¦» O¯?(玢'Ÿ?"¦» O¯?ïêEõòNÖ?j'—V§6O?eº
Á®?j'—V§6O?ïõHåÞ&ø?U­'r©W?Un4wÿW?U­'r©W?ïöÈÇ?6BŸœ ½?SÅü fð¬?6BŸœ ½?ïýùwrÎ?+XàFíiŽ?04DÖd7À?+XàFíiŽ?íè?3?"pÅ·pj?‹›Äx1Ã[?"pÅ·pj?ïóüë3ÑO?b\g (÷?X)'Þ?b\g (÷?ïÔM9ĝ?cŠƒh3&ê?uöYOßá±?cŠƒh3&êAGN4FGL J2153.1-0041?ìA5ÒÂ'ÀC߸ä¸{ÝÀ:é€æDmÀ<oèPïÝ@!æfRDpr?üÿüB?Äݦ¨ É?xCGŸÉ*ù?¶»]û)@txÍÇ?ïêLÚ¤%å¿ë^°ô)2¿œ›œNª³¿×«X¾ˆ…¿ÛoŽ˜´—L¿²WxÅ8¯AGNbll3FGL J2152.9-0045RBS 1792?ïþǾ•v?(v¢
R?#"#/ø¥|?(v¢
R?ï츘{¹?h±Æ¦3A?cGgÏÈVÓ?h±Æ¦3A?ïî/‡pæâ?qÔ_èÛ?aÐx"˜~>?qÔ_èÛ?ïû¯;ŸñÖ?,ų·úd?AC+]?,ų·úd?ïýëH–z^?0ÛqüÏóŽ?0¥¼±"n{?0ÛqüÏóŽ?ï¡$éL?‹øºð?‡¶ÅŸ=Ø?‹øºð?ïðHIgIˆ?jd^þ?_olÑ7á0?jd^þ?ïöÿx›*?EGØîhš?R3ù{‡?EGØîhšAGN4FGL J2153.8-1137?ì…?RåÀFÏËÉdcÀ9JÃÿž±1À<çq"Á@Øi¼\<A@7bR¯'?­'n®ßQ	?° ½ ñ
?ü'*߈'@›†é_¿Éó£»±q}¿åcn.±Ä3¿çBE¿é}þ."¿æà+²~m¿çÓ`žü/AGNfsrq3FGL J2154.0-1137PMN J2153-1136?ïþÅj­ÈÑ?ä$×ÒV?#©R˜‰Ç?ä$×ÒV?ïìbv99ª?gJüÝ'º?c‰Í¥Ž?gJüÝ'º?ïæGÅïìj?qïð?i¸: 'µ¿?qïð?ïù&‰£ú"?7û«÷
Þì?KeÚ깦?7û«÷
Þì?ïþ`é#ðu?"­G©¶3?)ñq­ìÏ?"­G©¶3?ï¢ß«¡®ç?	\ߤÍ?‡H(ÂR1?	\ߤÍ?フnI?ðÏ=ÆÜ1?€\äm¹} ?ðÏ=ÆÜ1?ïå-0º²ï?\¡"¨2ô?jÒÏ>mÙ4?\¡"¨2ôAGN4FGL J2155.3+6602?ì>\Ò=úâ@"	¶o"5ÒÀ:êg¹MÀ;²ÎºÖ¨@Iß,ö®@p'ݽ¶?ÉÅ?º«3?ÈóÜ܉0@γ!*3@Ý:ÆF¡?Ë*é£OA¿ã7ÊaŽž¿êdkð"ò¿å¬"½ð¿î÷à†=¿ïÚÀ«VZ€AGNbcuNVSS J215520+660839?ï¿E;"?{¦²1B#°?€.ºÀ=Aß?{¦²1B#°?金tð?ˆîYû¤³?†þbøƒñ?ˆîYû¤³?ï–ÄTÙ B?ƒO¨/Æ®†?ŠNê×v_]?ƒO¨/Æ®†?ï(~–;Ÿ?y©œÝúÿ1?šî+€¾*?y©œÝúÿ1?í84/:2ß?¶¤þSÏØ<?¶>^‡æ7?¶¤þSÏØ<?í#ùj Ãì?»©'£mì?¶à4©°%?»©'£mì?êmGoð?´¨Åí-Â?Ç߂Jâ@@?´¨Åí-Â?ç—LlŒ'—?°ˆÔQ/ÛU?ÐÑg&æÚÑ?°ˆÔQ/ÛUAGN4FGL J2156.0+1818?ìR%|'KÀ;Èf^ê–À9æ7UãUÀ<-5Ã0l@!ŽsöœÕ?úP¿54•3?º‹ÉwWÐL?¸š¾²­¼¼@:g9Êüé@ù0´¨¾¦¿ê?ßÿY'í¿ÂI#ŸíE¾¿×yTŸêk™¿ÑBõ"ûƒ¿Þnê.£ˆ¿ÒÕ½aIñçAGNbll3FGL J2156.0+1818RX J2156.0+1818?ïýŸ¯1?%pöððÓ¯?3T1"?%pöððÓ¯?ïåZ½Ä´?k"v.Ügš?j¥BŸUÓï?k"v.Ügš?ïï?Õ±€?j7W3iÂ?`Àâb¨>?j7W3iÂ?ïßΰã?Té©%\?p§ÆúK?Té©%\?ïù	HÔO?Dù:é¬þ?KÚݤ7{?Dù:é¬þ?ïv€¨ô?" ÍÛ²~?'/êö¥Û"?" ÍÛ²~?ïÏþBe«+?'
*'uG#?xÞ¹<®Ó?'
*'uG#?ï"áŽ?yrâÇ;W?ŽÇ¼Ò	ËÑ?yrâÇ;WAGN4FGL J2156.0-6942?ãN¸Z'‹ÀDH—žÖÜÀ:T}á­.¢À<((@éÈ@rK'ÎÉý@Eþw?ƺøcÿXæ?Ôûñ}†=œ@3öÂiœ|?úpH»ÊF?À *Aò闿ÌĈZ¬ôÀ¿êôZ5Ö|¿ïýA©î{s?®-ýê&$¿ïûpÿqºAGNrdgPKS 2153-69?ïéåà!ÆØ?m—‹O'|,?fɛ€T?m—‹O'|,?ïQ,jº?¥MĤ¢EÁ?•Úr¬ä²Ä?¥MĤ¢EÁ?îOœPê9€?šœ¡Y@3?«:ôÌõ?šœ¡Y@3?ïÍ# q?k %›6O?ynpE"?k %›6O?ïrì–Ia?š‰<£K(…?'¾âfW›õ?š‰<£K(…?çÓ)NǨ?Ñ+Â]"g?ÐY­bp¯ã?Ñ+Â]"g?é],ÀA<û?´a
Û´&?ʋLþû?´a
Û´&?ën¢ê•?µÅ-	?ÂEtU‰Á­?µÅ-	AGN4FGL J2156.3-0036?ךQ›ºAkÀD+¿@OÂÀ9é Ï¨À<3ëGWL@+ót¡@ÜewS?µæD1?œöCW‡j?åB]"<@µýM?+¿è è½ïk¿Ø.}`ä¿æ'S‹'¿á' ¹Ée¿á~ˆÑË9O¿ê–ÿ5¿AGNfsrqPKS B2153-008?ïþwlü‹4? $cq?(‰/¡t? $cq?ïîÝol}?c¢"AË)?a"ïrVó!?c¢"AË)?ïñÔL⠍?b8;16µE?\Wf˜4D£?b8;16µE?ïÿTíJÏ:?*™g"ý?b\qϟ?*™g"ý?ïü¾·¶:9?7%2QŽ*?:
Am1«?7%2QŽ*?ï–`@Ã?Æî¼`Ãå?Šgù˃]?Æî¼`Ãå?ïëZð5º?qtOÚ÷?d¥&ÿ?qtOÚ÷?ïþoaG€?Pɤ4?)	ìvOqÚ?Pɤ4AGN4FGL J2156.9-0854¿Ôµzö–JÀF]xÀ:"¶ÂŸLaÀ<z™_·ö@œ¾¨Fۇ?üâqy¿ß?ÌÙäwä=,?ÌMbI†@ê̒@p"³¬¿ÜM[=…¿åÅý_çœ1¿Þd}§ö¿Ù)*›´üÌ¿àRh' Xпïù–m•/AGNbll3FGL J2156.9-0855NVSS J215650-085535?ïê€÷â$M?b ^ýõd?eÞ¢ãq?b ^ýõd?ïÜsš›;?qyÛFRr?qÆ2¡4e?qyÛFRr?ᅭQ¦»Á?wð¢!ÏôÐ?€k•I-¾?wð¢!ÏôÐ?ïΝ©7‹ ?['V^neÝ?x±+i¹Ï¾?['V^neÝ?ïʯèª<Ä?zF-46UŒ?z¨•"
;?zF-46UŒ?ïMÂhùF[?ž[!Ð"¦?–G²Û¯Ê¦?ž[!Ð"¦?ï	°(¸l)?"X2ÓK#?žÉúïѲÛ?"X2ÓK#?ïåØ{EŠ?†7¾Òë?œCDõ¾¸¬?†7¾ÒëAGN4FGL J2157.5+3127¿ïñò"œÀ2="ôÆæÚÀ8I"ðÅÐYÀ;¬šÚâ9F@_t;@_‹Íþü?¡aÿÏX˜?Á|®¼Áfè@ c7ë(Øf@xhZ†­¿«Íÿý¦´_¿à‰¶b'<…¿ã'7oØÕð¿åU¥ïqó¿ìž–XœyH¿êÒxþn…oAGNfsrq3FGL J2157.5+3126B2 2155+31?ïì»Þ°Ž?b[aÂÁá?cD!ב?b[aÂÁá?ï¸gP#âf? õÜ79W?æ+ð€$? õÜ79W?íµ
á?¦?¢Û©lGg?²WöÔ?¢Û©lGg?ïüS™ôÍ?5îYÌK?=c1i+ûB?5îYÌK?…ËAÄ?‡¹p…–Zß?ŒÜž—~c?‡¹p…–Zß?ëlm?·´.I@E'?¦'P-?·´.I@E'?îs4ùdý?žªæÔý÷&?¨Ì°ek;?žªæÔý÷&?ïððëºù'?Rn¢D—ð[?^(PSo?Rn¢D—ð[AGN4FGL J2158.1-1501¿ïRT7Ý|ÀH<ÈóÀ9G+ý´Ì%À<"?ø="ß@'€ vÃ@¼w¯d?­@
‡‹ã?±"\éü@]Á@ŸS²¯•.¿ã™*GÒ'¿Ú²Í\¿ž'¿ãž¯çÜô¿äRÀí ¿âi%'×µ^¿å-c ŽUnAGNfsrq3FGL J2158.0-1501PKS 2155-152?ïþ(¨¦ãë?;ÄԔ?-uxp:•§?;ÄԔ?ïìNÒöÝm?g™á"§BL?c±,ûd#'?g™á"§BL?ïîV¥±³t?`™³ïS?a©Z
ô3ô?`™³ïS?ïó:¼-\?CŒ7v—{4?YŠ‡ÑBÄË?CŒ7v—{4?ïûh1eT?:<Šup¸?B_;wkñ'?:<Šup¸?ïæŽ{®?'t—f…>?ˆ†\P
§?'t—f…>?ïݤlA­Ü?x;§g4Üô?q-ÉæJ6?x;§g4Üô?ïÒ@`‡'?g˜©‡µÚÛ?vßÏÑ"£?g˜©‡µÚÛAGN4FGL J2158.8-3013?Ûõ26ˆþÀJ&k¤"ÉÀ6A7Cc,À:p¢¨6@Y'¹'m?üDÄö>¶?‡Ñ)ëЍ?¤ùÖp9£æ@tBÇû­@ñé…Àè¿¿âÈ6ºý¿Ö—¿¤Æ¿Ü´žØ»g¿ÙÝF'vú¿à;`ÿX±¿ÛՀºûiAGNbll3FGL J2158.8-3013PKS 2155-304?ïæÚ\œ?ž|ç씽?ˆ†{×'Hã?ž|ç씽?ïçà?ñ2?w^õK û?háÆîE?w^õK û?ìêC˜[+?©|E1Àk?¸­ã<JÀ
?©|E1Àk?ïþ)˜©ß?#†þ†œ»?-f±)
?#†þ†œ»?ïöè¦`ì?bÄÈþ«Q?R.³raà?bÄÈþ«Q?ïtQ/6h6?¡"(ꥒÜ?'uÚÃ]N?¡"(ꥒÜ?ï,RnM?œ‹¼®"ô?šu½ë_>g?œ‹¼®"ô?ïýé*â'î?,f6ݱG–?0¶¨Ýc÷?,f6ݱG–AGN4FGL J2159.1-2840?Ç͍MA8ÀJ<³åuÀ:ŽF@RÀ<AôÚ2@ C¼¹Ú+Û?û<\ŒÈп?ÁDœg)Z?ÄX¾Š@BíJ.!@vðéa­ð¿ïÿülò?ïÿÓ?,» ¿ßep½Wcê¿Ôo……t¿ã#-A+ÄT¿äK"=,®AGNbll3FGL J2159.2-2841LEDA 3218689?ïû'5ÞD€?F(5Œ#?A·(»´Î?F(5Œ#?ïÜ_ÄV²?}w­Zqˆª?qÐr	æëR?}w­Zqˆª?ﺓ½ó§=?'Éjyfå?[þŠ®?'Éjyfå?ïÌH9÷êÕ?_'ǡ?yÛãw±Q?_'ǡ?ïð'·³h«?] %Ê ë?^úr³	°?] %Ê ë?ïEkÿ?«@ku²?—OÝÏ-Ä?«@ku²?ïz/Ð
…5?ŒžÅ¥ny?ºúß½g?ŒžÅ¥ny?ï?»v"}?ˆïÀp1¼?˜žì&t?ˆïÀp1¼AGN4FGL J2159.8-4751¿êö÷€—:ÀImÙ]ÔÇmÀ:zê÷Z?À<ƒdIU´g@t"aS×î@(?NÊhn?¼í™I'›?" ë!<¢?ÅËÀæå@¿Q$_Û³?ãÁ­Ÿ`¿ãà%¿­)™¿æ9Áø]tO¿é+f ïÀ¿ïýŠoZ*ï?ïßM œÃAGNbcuPMN J2200-4751?ïýþLîèx?0'‹‹°Ür?0
˜âå32?0'‹‹°Ür?ï÷9QãÖ?Uœ»ŠI¸b?QçŒîDԌ?Uœ»ŠI¸b?ïւ=åò@?wbDÞÎLj?t¾áŸÅ?wbDÞÎLj?ïÿÌ-ëu¯>ð'óøÓ>ùéþ–,†>ð'óøÓ?ïþsÇ^4$?-/­Jª?(ÇX§Ý?-/­Jª?ïØiðÖä ?€ÎWõC?sˍ®wú?€ÎWõC?ïÐõkL)?€K$ËÏ<b?w…uI©ÿZ?€K$ËÏ<b?ïÿhA4e?x¯£åßÍ?÷ÚKZîá?x¯£åßÍAGN4FGL J2200.1+2138¿î±BU˜–mÀ:>$þ½
À:-m÷T`À<KvY"±@.WÁ²èJ?ÿ¡mµ?¼×Õ˜8F?°R,—Õõ?ô'p*4†ð@)ˆh™Çg?¾†ýOüm¿Ý-£ùnì¿åœº¶IӉ¿Óú D¯¿áƒsR3Ñ¿ëwÁ½¥AGNbll3FGL J2200.2+2139TXS 2157+213?ïþٞ[9%?
4LFG@?"fÕ#ä†?
4LFG@?ïíÓé²ÇÏ?d$ít1)?b,ThÙ?d$ít1)?ïö'òÔ|?c•¿øÜ}Í?RûÚ¡·X?c•¿øÜ}Í?ïýh[¼œÜ?÷Z©·É§?4½ dd˜<?÷Z©·É§?ïþbHAÎ?#Øgß/?)Û}øîH?#Øgß/?ï›>ì
:þ?™V@NZÉ(?‰0EPx'?™V@NZÉ(?ï÷¬ê"BÅ?`M°f'Ü?P¦*Gæ?`M°f'Ü?ïújEL?6Ù7ÕT·?GšVr¶ÅÚ?6Ù7ÕT·AGN4FGL J2200.3+1029?ï—Çñ,
áÀA.@…+NÀ:x3|.NÈÀ<PX(¶¯@¶Z
'º@ISù|X@?Áñ"ÂÅ7?ž¾}‡Gåû?Ú¨Ë%WÓQ@I$ß]s#?ïÿûB«÷¿äÜ)áû³¿ê²îO'¿×ôè_Op׿éL÷?7á¿ïÿ¬)ÜrAGNbll3FGL J2159.8+1025TXS 2157+102?ïíò‰a
?\ây}^–_?b
vø½;?\ây}^–_?ïÜ…Dë?vÆ3/B??qü½\—²›?vÆ3/B??ï¦Êm²?­¶HÒ?†M[ÖÕ	=?­¶HÒ?ïÒCI*ì=?]ÝWƒOx_?vÞ[Wûý¯?]ÝWƒOx_?ø'e‡?ŒøLØJÚD?ŽVìÔª?ŒøLØJÚD?ïS¡n¾éN?ž´otƒÀ?•‹Ò-J@4?ž´otƒÀ?ï4]˜j";?"åw ox?™tLë܀¡?"åw ox?îúÁ÷ s?‰¹à4S[×? SàŽøÏ?‰¹à4S[×AGN4FGL J2200.7-2414¿äÅP4SwTÀIÎWâ?$ÙÀ:•'Àa"À<'F…@J'KÇ~¯@e9Z"¡?Áþ{
ã3?©¤2|]?æá¤_Æ95@
Ô‡Spë¿çtî>Œ'°¿Öµt@™£*¿æu9½æÕâ¿Ùè<œh¿æ'Z«GA¿ä)~HÛ;%AGNbcu3FGL J2200.9-2412NVSS J220036-241428?ïþŒšOŽ?µIâwºÇ?'6YæÒ?µIâwºÇ?ïð_ÔÚjù?b"»ïEüÆ?_@V'¡îS?b"»ïEüÆ?ïffl>#ã?k%àќÙU?`S{¢
?k%àќÙU?ïýΪûõ7?Ú©³Ÿ?1Š¦ª"W?Ú©³Ÿ?ïþF
6 â?$Z§ø~–?+ŸYK¸	?$Z§ø~–?ï«tT?‰}©´ÖU?…"ú$¤H?‰}©´ÖU?ïñ*\Ÿé?j6{NÄK?]«G#ׅ?j6{NÄK?ïùlÇÕ?<˜ðÝúãm?JOÌRrÎ]?<˜ðÝúãmAGN4FGL J2201.0-5907?îâD'oÀGW}|,¡IÀ;:p>V}À<ñ8Ë@ ¥xJŸ?ýs¸ÿnx?Ô—ç—S?Üþ#[ú§¦@gGzÕ@:ԈØ׿ëU ÃÄæN?í®ðBóš—?}Ö¨¿âGò½¢7x¿éØb,E¿ºRÅʤÿAGNbcuSUMSS J220107-590639?ïñ·¡Ü"?]'ÕRò\$?\»äÇM?]'ÕRò\$?ïßG†&u5?'üVð?p\<ìy¦?'üVð?ï5æDÈ%?‹*õÄ_7j?™C7v—\?‹*õÄ_7j?ï¡níž~†?tõí°"±?‡¤D¦Î|?tõí°"±?ïžfFþ8¢?ƒÒ÷Ö¡)?ˆfn6#Ž?ƒÒ÷Ö¡)?ï¶Ó¹{d?‡¥ëÝ?S?'K¡=&ý?‡¥ëÝ?S?íRçŒd?£šòß*ÿO?·hßÜ?£šòß*ÿO?îØýÏ4l?•ûÒC»2õ?¢~°Á6A?•ûÒC»2õAGN4FGL J2201.5-8339?ïäÝüÀ?¶,ºs-õÀ8¨á¼©iÀ;j¥P‡@ž«"‡@î.|M•?¨ß T« ?Âü]CÆS@ï»@ãÑ C—Y?ïGòrxÃ`¿å&H.ÿæ]8TÛ#¨¿ç÷#b…±/¿ëãIEÄ/o¿ïþâ=ø3-AGNfsrq3FGL J2202.4-8339PKS 2155-83?ïõÕf?O¶üV1(?UÀU{u¬Ö?O¶üV1(?ïòTó›Õ?b{¯.ôb¨?[VûÖÏÖÕ?b{¯.ôb¨?îØØK%?›R¢9PX³?¢sÃHÏ°?›R¢9PX³?ïùÿQÿZ?5ä>«¸lâ?H«T°È?5ä>«¸lâ?ïákÈX?i.
'íÀp?næ"xOr?i.
'íÀp?ïÌC	6ê?'ÏŒFXœ?yÞ{H'?Y?'ÏŒFXœ?îÁ÷KÀ?¡6Œ.!%•?§ãà‡ç*÷?¡6Œ.!%•?ïÛã¦æ'?cïXÙ-è?r}wG?cïXÙ-èAGN4FGL J2201.5+2950¿ìۀ¸]eGÀ4ë9Ÿ]ÿÀ;×gZ'À<ˆ~aßï@@)iÛ»Ó@^ø³Û?Ï7‰I`œ?¶¼¬™%«`?ç¬ÄÉ$¢@k—ˆrTÜ?ӇŒü¨1¸?ïë뫵%¿æ⤥fVv¿×–£EG¿êaQžÙ•?¤,٧ѕ´AGNbcuRX J2201.3+2949?ïÙ¤˜óxÕ?­˜M[€ï?s-³ifÝm?­˜M[€ï?ïçóª ?n}É/çÓ?hà6C"Ì?n}É/çÓ?ïÓ~½Ó¾6?tՊ
'?v@¡ DÜ?tՊ
'?ïà"œ»?Qž°å§˜m?olᄄ•‹?Qž°å§˜m?ï÷ü6­ø2?JÁ­ÛÒe?P'2‰RI?JÁ­ÛÒe?Öv'#?•ÿzZJ_†?Œ_Ês‰Ã?•ÿzZJ_†?ïÇõY€FY?6¶@àm-?|SHãŽ?6¶@àm-?ïmœ<Ùq˜?'ÄŹª}?'Lxiù6ñ?'ÄŹª}AGN4FGL J2201.8+5048¿îᢃ'ß*Àdg`ai§À7²š²žM^À;L(Ê#¥!@¶Ý®òFY@€_†xT¥?›öAô?Â4J@Qü£T-@ ·áXJ¿Ôy!Ôæø¿ãyk@Àºp¿èÊ÷uR¿éñ‹@;¿ì¥2Ÿ9–¥¿ïÿ»!(ĚAGNfsrq3FGL J2201.7+5047NRAO 676?ïî~u®?_{
²€ý?aäŸúE?_{
²€ý?ï"ã&t'?®ïò­Z_?ŠÇ²ó?¥?®ïò­Z_?îô
!}9x?—ç•Šr2˜? ¿]ãàå‰?—ç•Šr2˜?ïþO~mnB?#Zaî'?+0žâ?#Zaî'?ïٜ½Õ&ý?q|¯
"|?s1¡	
éw?q|¯
"|?íù·^{‹g?ÀL&?°2EG½Ì?ÀL&?ïQkNúÜ?™zr˜ëø ?ŸÕҔhÖy?™zr˜ëø ?ïø};ƒÓx?H²?Ú±6g?NΧØ?H²?Ú±6gAGN4FGL J2201.9-1706?êð§5A3ÀHØ#|ÜÊqÀ;Í¥,tÓÀ<Òï ´«n@$/ÿ¨Â+‰?ö…6+‡?à«úYÍÑ°?–´3<²&È?¬ÊÎþÙº?þ¶ìM›"F?çøäb•¡g?ÝYŽÏ[¿å>^‡tÔ¿ïÿZS2¬û?ïþSW•é¿Îîì\_&AGNbllRBS 1813?ïÿHÅ
2:?s†T?çbÇ'$?s†T?ïêË\דÈ?ty{¸¦XÔ?e4£ΐˆ?ty{¸¦XÔ?ïti5ž}?
â‡Aß?'rÙU5*s?
â‡Aß?ïÿ.«'û6?Ä~ðl$$?*'oKÓ?Ä~ðl$$?ïþY<1^?2"?*l>b¤ò?2"?ïœÊßjfÚ?†œ˜¥Ék?ˆÍH!ö­˜?†œ˜¥Ék?ïJGêƒ?'çûàRŠ?–¿þs"¦?'çûàRŠ?ïúpÈÙ¼ä?NéÙg'ͨ?F<Ýpˆ-?NéÙg'ͨAGN4FGL J2202.7+4216¿³r°Çi©À$ãb¥ç…¶À61â§)¥À:¤Nér@¸¨§ÿc@%@FA,ñ?"•1f:­·?®Õ¬€?T@$YH¾H¦@ UšSÓ¼«¿Ä¿('!-¿ÞýÀà…f\¿ãӉX=¿âÐíޕL-¿æ;a3v¥¿å(ê¥$èAGNBLL3FGL J2202.7+4217BL Lac?ï±2MÁ:.?³Îõç"c'?ƒ³l"È£?³Îõç"c'?ïsTSxX?«NË
[½~?'•uõ?«NË
[½~?ïŽ ¹!ãï?Ä—ʧS?ŒwÑ´h4?Ä—ʧS?ï÷8=´œ?MÝ~5é§?Q…HçÞ?MÝ~5é§?ïêŽ>‹?eMÅ %¬d?eáýªB?eMÅ %¬d?îyWYÙ?±–ÞÝ;G
?¦øj‹>V
?±–ÞÝ;G
?ﺇՙF…?‰ªG=‹Ž¯?^
š¶@Ä?‰ªG=‹Ž¯?ïÌN¨¿¨?syõõÈ$?yØ«Ý#ì?syõõÈ$AGN4FGL J2202.7-5637¿î'ÃH¶õlÀHÓþuóÀ;WçS`Ð$À<ג:)Çz@ —½çו(?üì*EMçê?˯ >#|?²t\É.²›?è|îh(?ûÊòìq-?Ú¡Ü>ñ§?îÌ Ÿ²¸O¿âsÞ-è¿Ï¤Váä-¿ïÿò~#¿?ïÿ·ÀÌ
ŠAGNbllMS 2159.5-5649?ï÷ӔÎ>ù?R!){
?PX֋£äD?R!){
?ïꋁË>?p`¸§#äl?eùt–ññº?p`¸§#äl?ï@Mž!a?j‡+"?—öL3Eå?j‡+"?ïâ'>E#å?YØ m~ͬ?mnÁ¶¼'´?YØ m~ͬ?ï÷§zi
ò?Vê'ÐÐ?P±-ä}?Vê'ÐÐ?ï²V·FÓ¤?ŽÙg••ˆ?ƒjR8ñàñ?ŽÙg••ˆ?ï€ï>;Ïå?êŸš$?Ä0mœjÎ?êŸš$?ï}¶xü?"2\úO"?I=Ær?"2\úO"AGN4FGL J2203.4+1725?l‡	AÀ=£µ¿j
»À8:²ái<À;§I׺f™@•äô¶Ë¯@ÚŸb0w?œý( Ëß?³"a†q@ö_½Õ¹@ebÉ"ô!¿¾¡O›s¹`¿ß:ÆF¡¿åK~îóhB¿å7_ÞO¿æ¡!þ'|r¿érR,ó~AGNfsrq3FGL J2203.4+1725PKS 2201+171?ïýRI+  ?+½\ëlë?5m¶P"]å?+½\ëlë?ïêå<Š?gµ¸ÇNä
?eýéñ'û?gµ¸ÇNä
?ïã}V¤ê?r.&†¨T?l'©þ—¦J?r.&†¨T?ïÿ¤îar>ø§·¬Ü?ÄvíÀ2ñ>ø§·¬Ü?ïþƼ^âÜ?¯Óµƒ"¨?#"6PÙ!Ü?¯Óµƒ"¨?ïzÀÿԋ?¡}ÿ96?§à$¦Š?¡}ÿ96?ïò¿?›vi?fT5?´—=?Z€µÕ^÷?fT5?´—=?ïÿiÈy3¦?
*>û։?ÆøkRº±?
*>û։AGN4FGL J2203.6+6751?ш8U(rÝ@#ç@š$À:[¤ˆ
%À;ÚVų-@å‹
µ'@—Ö›'§æ?Ï"¸ß/%?Ç¥ÚZ)O?ù Äeõþ@5àŽ5?íõ«gᑿèÿ|'1ž¿èсèM¿é¾x`¹Ô"¿ïö¡÷6-¿êÐØËЯAGNbcuLQAC 330+067?ïÛ¾TŽø?{Ÿ™˜ég?r ÕØ 'g?{Ÿ™˜ég?ïWœñµ0ñ?š¦R!¦g	?•aÀÂÛæ?š¦R!¦g	?ï]Õ͸–?‰'×r1°?"^åH»5?‰'×r1°?î|˜&5?‡$ÀͼÁ$?¨6Ûç°?‡$ÀͼÁ$?ïx‰Ôžœ?ÓõŽv¡?îÅnT^Œ?ÓõŽv¡?ê§ù¦!?Ȧ¢…jQ?Ç¡`g§{?Ȧ¢…jQ?éÆüB¨"?µG€b|*?Èäõ]²?µG€b|*?ãzVTÂÇ?²‰9
sÞ?ØåSVzq?²‰9
sÞAGN4FGL J2204.3+0438¿Ñ°ÃáZ'7ÀCT!BoçÀ:
,·îïÀ<Qé{Y<²@ÖIGF»{@­|ÀDÿ?»"žñ-?¿ÆÕfú5?þ`Î\‹@Íêæßó¿ãӕ:a%¿âôÇÝÏ©v¿ãiÇåv¿çôÓ˜A¿æZ1¿•¬¥¿ænnD—àAGNbll3FGL J2204.4+04394C +04.77?ïþ
–~?Ù½=áL?(#¿ëß?Ù½=áL?ïè
œ¬?ko®Æ÷Õ ?gòd(dP?ko®Æ÷Õ ?ïòÛ]øó`?\w¼Ä¨ÑD?ZICÔ_Ð
?\w¼Ä¨ÑD?ïé/u'?L쯳ëž?foå¥`Z?L쯳ëž?ï÷Ÿè×ß?Q:*²Öãn?PÀ.γx†?Q:*²Öãn?ïƒ0.È?'º,ìZ!X?94ƒ!×?'º,ìZ!X?ïÑÚÛÆ?|â
g?wþ&
|˜?|â
g?ïz´÷ß?{ÙMÛø[=?©a/+?{ÙMÛø[=AGN4FGL J2204.5+3634?Í9\ÇEHÀ.\ÌîZ¼À; È1\™^À<J'Œ"Þ!@ <7"À@§äRµ?ÅÑY¹Ú¬´¿£§àYF˜?â"Jb#á‡@+
s†	š¿ç|'ݽµÙ?ï·õÿËþ¿èÉ[]ô§Ý¿ås]û]Ùпãõ
}ìêÏ¿œkÊÃ!?AGNbllMG3 J220423+3632?ïþpQ‡î2?%»ijŠ?(úèÚ\	^?%»ijŠ?ïìÖâIÎ?kÓT Ë"?c)àWšy?kÓT Ë"?ïò6B©•2?Tz_z'§?["zx›?Tz_z'§?ïøî«fB!?4°J£œ÷?LEQ†ÛL?4°J£œ÷?ïýo²Èó,?/ÂÊ?ùë6?4'h†¼"^?/ÂÊ?ùë6?ï˜ÐFm¼?•¨€ÂQ+"?‰üõCÈÞ?•¨€ÂQ+"?ï쫝ä==?naNtPz?cTb&Á'è?naNtPz?ïÍ/QëôÊ?p<6:^²?yhW(òÒ?p<6:^²AGN4FGL J2205.0+7432?çî0Ïå@.dvò¥¤jÀ:å*Óa,À<ap9N@xs²Ì›@ùš‹1!?ßš"Ñ
Ÿ?è…ë1;â.@l Ÿ²¸O@¢ÊšÃe¿ï}Ë<©Ôz?ïÿ÷œ"/¥¿ÎI‡9£¿é1ÿŒ<¹Å¿ìËÃAe%?܂›üu¼AGNbcuS5 2205+74?ì|"åB‡?Ⱦé½ÑåÄ?¼߈ÕëÉ?Ⱦé½ÑåÄ?ï‰@¨ç•P?˜*û½a[ ?¯Õ»ËØ?˜*û½a[ ?떊AH0?¨Šøšo¨;?Á¥Öúß?ý?¨Šøšo¨;?íünHÊÁ?˜ ³÷
Zn?°‹•K¶u?˜ ³÷
Zn?íÏÿx+ñÝ?¼Šæ&ÔÄØ?±€@X??¼Šæ&ÔÄØ?ëÜvCåCL?Ì5ó4žï?ÀŽ&ðjòÎ?Ì5ó4žï?ë!LŸ¿?«ÁÖùœD·?ÏzÏ݁?«ÁÖùœD·?ߦ§¯1†?Àr"A!»?à,¬(g}=?Àr"A!»MIXED4FGL J2206.8-0032¿ïH3®`ْÀE4Áü28À9Lå".(1À<ºß%•@r=Ô¡ØW@?› 'W?±g¨A
wž?³¯—‡Æˆe@šfH3u@c,°ã?ßüÒ¹u×ó¿ÜÛëc:âÕ¿äa~õÿK¿àA¨a2Ÿå¿í'C¿rq7?·ð©Jç…AGNbll3FGL J2206.9-0031PMN J2206-0031?ïü!í¡¿¿?67 §ÃòF?>ð".{''?67 §ÃòF?ïí¢»q•?eÌqØì]?b]E*Òæ?eÌqØì]?ïQQ‹…Q0?'ak4>g?•ÕΑ
¨?'ak4>g?ïûÃÍA3H?1@N4¥}ð?@ðÊg?1@N4¥}ð?ïøS
n'¦?JõÈÑÂÁ?N³Êc÷Áí?JõÈÑÂÁ?ï›ø3'äK?B'ÀŸQp?‰ó"¶‰ ?B'ÀŸQp?ïn,þ]5?ŽÎÖvˌ§?':`9€É!?ŽÎÖvˌ§?ïö&;™"?LV×X¾}?S³Ã3—lN?LV×X¾}AGN4FGL J2207.0+3607?¸+ßç¸À/°ÿŸ‡ðÀ;i£ÙŽÀ<c…Ò<xV@ 3
ž¤@IsÙìp?ɪ+¢› ?ž(Û@'üõ?Ö¡sÕB<@úm‡	¿ï¨P!ӏ?ëU°€æÅF¿â`‰ãC0׿éò"ý[
¿´t×~'¾D¿è '+"ØAGNbcu1RXS J220708.5+360935?ïþËò~¯€?	®x9?#@Ù9€Z?	®x9?ïí]_?i<‡æn?b¢þûþ¨?i<‡æn?ïê‡Z§ÁP?fr÷Á߈?ex¥BA0ˆ?fr÷Á߈?ïü*ªÅÞ>?+îÔ
»C?>ª©¾]¿?+îÔ
»C?ïû7ÀzrÒ?A¦å$»h?C þÝÄnÛ?A¦å$»h?ï¡u3fgq?""ºÙ=?‡¢³Oâ?""ºÙ=?ïáÏ;D­7?uÊúÌ|?n0Ēy?uÊúÌ|?ïæÈVE†ó?c<Ù¹æ•?i7©†>ý{?c<Ù¹æ•AGN4FGL J2207.1+4316?펙•Š7ÉÀ$FÎô©‹À:"qDúÀ<	Ÿ)üRÌ@ ¡™Ê–çŽ?ûèQÃA2Ð?ǯI™§"?ÐÐÉ<qu@v.	þ†ƒ@	n(Ãm¨¿ï²¾™-c?ç'!þW‰T¿áeHŽå
±¿Ù¤þývŽ¿Ó-eÿ8Yä¿ïÿäë8AGNbcu87GB 220504.7+430144?ïût
 ­}?9»5 ÏR–?B/ÊèN/G?9»5 ÏR–?ïæyÐN?qYÒ')b™?i†úSmcN?qYÒ')b™?ï"ø6KÛ:?‰G¨èY?ŠÁòbº]ª?‰G¨èY?ïêÝUÓh•?L"ÆJ7¸÷?e"ªüC…?L"ÆJ7¸÷?ïøDYm¦ï?IØ»ú'ò?NîšX?IØ»ú'ò?ï‹èH©<$?–õn'ê/?íÕ°÷?–õn'ê/?îâ6>^8?—SH/!^R?¡ÜœÓYŒ?—SH/!^R?ï¦/ˆÈ?xyÅ0«?†y>…KÙÈ?xyÅ0«AGN4FGL J2207.5-5346?éê½ÑÀHóþ®û+À9yÝ÷vÅÀ<j'¨
У@oPk'kT@P.Ë?«¢•Ûc?žù
¦z ?íã™BÞç@§¶š0m[¿Ú˜Ïö¿â[ýÂ8T¿æ¼ìOIo¿å—,×Ï_¿êú³fÊ9¿ÎƘ*XÄAGNfsrq3FGL J2207.8-5345PKS 2204-54?ïþ6{+[?"ñ…´¹q?,˜N4-n?"ñ…´¹q?ïöµ€l2?Vº³Àm`.?R•ÜžòŒ	?Vº³Àm`.?ïÝ!£`9H?tÛcõ½?qo.;E´?tÛcõ½?ïÿxVò"?w©Õ€ð?íùÿB¨9?w©Õ€ð?ïþYÅ¡½Þ?##µ¶k?*c¦Ëß?##µ¶k?ïÜz:r-?}é€dW·?qÂãó?}é€dW·?ïØ_ōh^?{¨ÛÙí‹ ?sÐXè8ã?{¨ÛÙí‹ ?ïþå}ÜØ?!ýªéb?!¯÷¸¤ãD?!ýªébAGN4FGL J2207.6+0053?ÕŽ]ëÀD×ú~¶¿DÀ:±Öv™ºQÀ<Uq€Ø@æ«͏À@ÂCÜ΢?ÄàĦbªÅ?¢ñ·¤ã–?ÝeêÕÌP@â«¡.
"?ïîÎ_¢¿ç0Èè#¿æfA¬Ž¿ê}ÅB"пÊX‰m~¿ïÿwD;ÏAGNbcuPMN J2207+0052?ïþÕ:¯~]? 5*?"¬W¯™³ì? 5*?ïìKæö»?iA™yúr?c´aJÔ­?iA™yúr?ïñ"2\??P;•Òl£?\÷š—Ï¡µ?P;•Òl£?ïþ+´¹°?k˫Ŭm?-D±®Ë/?k˫Ŭm?ïþ•û2Š?$6уJ?& LÀÚÎ?$6уJ?ïžèþ±¡M?â 9?š?ˆEÀWH«?â 9?š?ïæLõ8?n<æÃ>?i³!õ‡Ò?n<æÃ>?ï÷?9·î?GšI¶º»?QçBX"À?GšI¶º»AGN4FGL J2208.1-4507?ߒ'+·ýÀJ|ÁÁÖυÀ;É7PÏ%mÀ<òrâu«~@!ï0ì\?ü"þ_
?ßÓp?ƒ"µ?ªW[AÖJ`?ù²v‡›À:¿ïÿæ4|ßO?ïüv¨ÓÉ@¿ÐeºD	Y¿Ú::c~)§¿Ü˜bŒè¿ïïM•µ‹AGNbcuPMN J2208-4509?ïÿ?ùóª?"ËÕøÛ7?ÃÓ><S?"ËÕøÛ7?ïò_Zoç?bŽêV?[AL1w?bŽêV?ïÉý/s¾œ?€=Ù6âõ?{h("?€=Ù6âõ?ïùn¥hôz?8û[È¥?JEiÉe/7?8û[È¥?ïÿ‰‡£õ?çcC7i?
ž/pãÎ^?çcC7i?ïIJȥÜÚ?Œ:5Ri¦¯?}¦›¼/ÚÝ?Œ:5Ri¦¯?ï½ÊÀþ'?ƒä?†Zÿ?€Oýþ1?ƒä?†Zÿ?ïçmBVDc?_y‡xØJ"?h'½ µ)?_y‡xØJ"AGN4FGL J2208.2+0350¿Óˆ–%Š—ãÀCõº² À;RӘ˜èšÀ<«ÏèàÿŠ@oŠD¼óf@ᇿ}?Ìb~dßӐ?¿¶œ´¬?òÞU‹Lϼ?í¥ð¼¸yü¿îÛ
F9 ?ïã>"¹…È¿à"ä0– Á¿ä!Fkõ ¿áz+ª¨µ–¿ïÿCaԆUAGNbllSDSS J220812.70+035304.6?ïö1´ûAL?xmS	¦=µ?Sœ–üÈj?xmS	¦=µ?íñ`	CÃ?¸0Ò8è?°tÿ^lj?¸0Ò8è?ïmPo{…?ŽÇ:š8X•?'\5òV?ŽÇ:š8X•?îƒOÖ,?ŠÈ‡"zr?£×Êÿ-¢D?ŠÈ‡"zr?ïÏ&V©?ƒ,Lz¾<?xvlèég}?ƒ,Lz¾<?åŅ€æw÷?ÑDD`Š·Ý?Ôtôþ3?ÑDD`Š·Ý?ï-žÔ¹M?–Öã½|?š\ì' ¤g?–Öã½|?æû Îb=?¸$¦<¨…?Ò¿Ôc;†?¸$¦<¨…AGN4FGL J2209.4+4329?ïêuë‹÷À$h'­ÄÉÉÀ9ºÆîj¬À;›Wëy`>@˜%ä@|dý°šg?·¶ böð¿¨*£dÄ?ñ`ú@jµ§l@?än.¡©¡¿ènÓr'¿åHNöÞ¿é¼ÿ¿ã¡Ö^ÆßοÚÒÁÃÚ4êAGNbcuB3 2207+432?ïþV9Èxª?W[:Óã7?*œd'ŠNe?W[:Óã7?ïï*xW2J?oGkÛ?`Շ§mÞ{?oGkÛ?ïíN¼Èë?^è]‰4|ø?bâ±LÕüå?^è]‰4|ø?ïî)­£?C^·ØDóá?aíëÐÒü¡?C^·ØDóá?ïúÑ9îä$?@"k÷
×É?D»ÇÓ³#?@"k÷
×É?ï¨î}v£?'[Vµ:×?…ø"dó)?'[Vµ:×?ïÕ¿&ñÜQ?y'¬fVq?u l~"Û¥?y'¬fVq?ï:!'Ü­?zðOs.Ŗ?»×"Îo?zðOs.ŖAGN4FGL J2209.7-0451?ã뵊ˆQÀFÅ£~õ©À:aµÁŒäÀ<JO¾"4®@ âóÀ×v?þD¸)§™?·V3M÷ž¿¤"4áÅ=ž?îRàw¤|@ÕºåÈú¿ì¯©Ggž¿Ø†d¾E s¿ÏöN»ÏÏa¿çȧ¤WÚ¿Ô³çƒ?´æÐÙ÷­¡AGNbll3FGL J2209.8-0450NVSS J220941-045111?ïûéG#Lƒ?6¥èm?@Zâ°½Ÿß?6¥èm?ïêÞܪ÷v?hëÔÑÝê?e!#~Cٝ?hëÔÑÝê?ïÖR2/…²?všvh†	?tÖæÙÞø?všvh†	?ïõïØ{y?@÷*—êB?T Pa},«?@÷*—êB?ïìädK¸?aÉ_=}èý?cþ¦³Z?aÉ_=}èý?ïmMá4c?•*Y7,P¼?Œ$¬‡²çH?•*Y7,P¼?ï¿)ßU>?ƒCÑ#F?€5ˆ7ˆt?ƒCÑ#F?ïÍÜÖ‡?m¹}ÉDv?y"Ù¿š!?m¹}ÉDvAGN4FGL J2209.8-5028?Ý,›úqö'ÀIƘÀ¤ À;Lï͂Õ2À<¤u‰ïØk@ÖÙyÙ_Ø@œ÷S½?ÐÉý·{W?±äØfÌh?ã´£
[£•@Úºch°?í«ñŠò6ê¿álÓu]¿æÂIá nu¿ßmA£¹X¿ë®Íb¿ï÷9R1%<AGNbcuPMN J2210-5030?ïã)É/¼å?¢5ÿôÊö?lÖ6Þ‹B?¢5ÿôÊö?ïöLÓËÍ?Vê÷î®/é?Sófš`åX?Vê÷î®/é?ïÔžg½1?}|'VhT?uû°Èßp?}|'VhT?ïýç­+z`?òi­Æ6?0–F·¢)?òi­Æ6?ïþèÒ"2k? q"Ö¡[L?!rڇ ¹0? q"Ö¡[L?ïܟÕÀ2Ø?tM`nŸVÝ?q°þ:h<?tM`nŸVÝ?ïÚrÍÛs6?}ƒ§®öô!?rƙ'"ø²?}ƒ§®öô!?ï÷¦¢ç?BÅø¸Õ??P³Ü»Ø2Ü?BÅø¸Õ?AGN4FGL J2210.8+3203?ì'p Ú‰,À3Í_™Ã‹À;ÜjžÚK;À<ߧ[#<E@$œ^o÷à?÷&ª>,‹y?ѾÇüX€ ?ÂZ<¡ñ×É?ñÑU¡Îò@"ì3D{¿ïÿÿÊPË?æ´yï°&¤¿µ"¦:'ÌF?ïþŒÝôgp¿âüvÄ¿Ìp÷äÓ~ÃAGNbcu1RXS J221058.3+320327?ïþàÁÝk½?Ÿ€ìr?!óދzG¦?Ÿ€ìr?ïæ뚺£?pë
hìþ?iâ"s?pë
hìþ?ïÛ¶}2¹C?z¼½ÃÁ÷Œ?r$Á‡Ÿž"?z¼½ÃÁ÷Œ?ïó{5g&?Q!>1¬?Y	Ïý¥Òù?Q!>1¬?ïý±K'ù½?/5#YõgD?2u¤kÃ
?/5#YõgD?ïŽV½Út3?"—û†_f?ŒjP…óWM?"—û†_f?ïÙMð_	a?{Uû«Ú©?sY´Nƒ ?{Uû«Ú©?ïϪ×Wü?whô_1Ė?x*òsWÂ?whô_1ĖAGN4FGL J2211.0-0003?¤üßp/ÁMÀEy¥q"À:ÆîᵒÀ<tÌežÀ@ ZS6Ñù?ýP"{rg&?ÊXyÿ…V?»?äq"&Á?óÂíÖ1Ð]@Òì؅è?ïÕ1U¡Ï¿æŸÿ®—¿Ý‰9"ÛòZ¿ã^M"0ÉÌ¿ÂaÉɍ'E¿ç]Ä×5AGNbllRX J2211.1-0003?ïýSË?B–²yGٓ?7Å_'Ô2?B–²yGٓ?ïèoBX>?jC`KÊüº?g½.'ý?jC`KÊüº?ïáðíè¯?w|ñj(yY?nøKÐÀÒ?w|ñj(yY?ïïžõè¾µ?Gþ6ç<ò?`a	åÆë¥?Gþ6ç<ò?ïù‰JZÛÝ?Ut­•¾²r?IÚ՞F%?Ut­•¾²r?	£(?'.{M=ó?š½"Æ\J?'.{M=ó?ïÙSû¢½?Xß5ù?Ö?sVMߝ9?Xß5ù?Ö?ï³Î¥%O+?uû
?ƒV­½9E?uû
AGN4FGL J2211.2-1325?⟝1Ý%hÀIÌ>1"÷À:ŽŸj"óÀ<U¢šÊB@§"å¡ì@™f`‡)U?ºöÄBÃ<?¨æª"xu?ßÁ6+57ð@Ó1p:z¥¿ÄnÖ·Ý&Œ¿ã[	pÂ	û¿ê֛'§å¿ç‰âÂW}ë¿ïÿåþÌú?ïÿ}Ž¡AGNbcuPKS 2208-137?ïü'ã¸?6*ý	:º?;pçpd4?6*ý	:º?ïîWÓç?g=¬orq<?ar¨5¨Ã?g=¬orq<?ïÛ_bÚ/?kå'Jn?rP}IÃtµ?kå'Jn?ïþ®íFr‰?à©ëehê?%,½OÌA?à©ëehê?ïú¯Ì·?H´ý3qˆÓ?GÃá0OÍ?H´ý3qˆÓ?ï¡ÒÜí?Ž"¶È×ßJ?‡‹Hò,ð³?Ž"¶È×ßJ?ïÌl^f×i?{ÿ¡ÿ ^?yÉÐãA·:?{ÿ¡ÿ ^?ïùï¤Vû©?A7ƒ?HAn˦tï?A7ƒAGN4FGL J2211.4-7040?Ú\®j͛ÀD~	VÀÖõÀ:÷Óc¿ÂùÀ<À!ˆæÃï@Šˆ¯'@¢P¨­?½¬/ô9xG¿¨•Ú¦‰¨?ìUÐììýÅ?þ•'¦8
Ž¿àr·B!À¿à-YÕ^kƿ剀Fâ<¡¿ã¿ÕØå	¿à­á¥!¿Û¡œ1úNAGNbll3FGL J2212.3-7039PMN J2211-7039?ïýÚRé©?+d‡Ò'?7/7—¬Ð?+d‡Ò'?ïó¢Aˆá?`=ÈW¬ô?Yü»˜k?`=ÈW¬ô?ïë"øš'€?e.å4'pð?d{N{'±?e.å4'pð?ïø rJº?50Œ4¸?O†ýKSÈ?50Œ4¸?ïö¥ ­Â?Iä#Ž:‡S?RÞµP°üË?Iä#Ž:‡S?ïÇF1q?"QH­zð_?|\ç0ÙJ?"QH­zð_?ïä[¬?tE‡fð³µ?k¤S½‡‰?tE‡fð³µ?￝²-V?rŸ$u'z?€"Êîm?rŸ$u'zAGN4FGL J2212.0+2356?ëçÄRˆlÀ:q£±JÀ96ÁU FÀ;㶇*@´¸­@óŠ§ß­?¬ç…›ñô¶?¸É»{Eq@Á _ò@Ó/m¬¿Åº™™n¦|¿Ý7zU0³ý¿âÉUÐ-¿ä×àŠ"(¿æQßp¾Y¿à—àýy½AGNfsrq3FGL J2212.0+2355PKS 2209+236?ïÜ>]"æ?k‰:ø‹®Ö?qàÑX!%&?k‰:ø‹®Ö?î-å²æ‹?²«@?­!¤Ïßz?²«@?îüSWb^ç?":ÿ5w? :ʍI­ˆ?":ÿ5w?îg˜ô
Ý?Œë«|t?¯™†t.î.?Œë«|t?ïpÞˆ?Ž§œ,?$ã?'ä"Pw
?Ž§œ,?$ã?àðŽZÌ)d?Ñoï꼪s?ÞãJg­8?Ñoï꼪s?íZü…¢ê?£¥gú'k?µ(Ó]D0?£¥gú'k?ã¬
±]Iv?´Ü¬Ÿë?اäEm?´Ü¬ŸëAGN4FGL J2212.2-7251¿ïgŽð{Ü"ÀCËØà†8À:ùÊd<À{À<"+¯±3@ˆºÏa@¦T…"RX?Ðkcü(Úë?¶å¸åº/?é¢Nt@fãr«™ ¿çò/ýô¿æ\°ožôL¿ä–_'‹¿ç!·à¬~¿ìì¿B ¿ïÿA(¿;ëAGNbcuPMN J2211-7249?ïüM¶l87?:\a쪮?='NQ¦[F?:\a쪮?ïõ[ʉ¯?XåÔ«Ìu²?UHk ÛÒÚ?XåÔ«Ìu²?ïÜ7Ža­?p$˜#‡—?qä8·/?p$˜#‡—?ïù‹"?1æÝXÕ?IӁ¶:Çw?1æÝXÕ?ïýËÄLK?*'`[jf?1§/ùÔ­?*'`[jf?ïÑùNNÜ?'óÞa²;?w@e7)É?'óÞa²;?ïÓíÓáÂ?|kCÏÉe"?v	0Žÿ?|kCÏÉe"?ïÕc4éÒÓ?h Ÿð'F;?uNeu…?h Ÿð'F;AGN4FGL J2212.6+2800¿î*0•Ÿ#À6ülü'œþÀ9ëÕYcH¥À<O'h˜p@™õ *­S@ãøÀpø?¶t·7_?³ÛÙÚý<+?üüYÒÚ-@X±G
V?ïäC '?à¡
+a­š¿áÑ0ߛÜj¿ã•"ÁËçÊ¿ßÛڜCB¿ådÏÝùDûAGNbll3FGL J2212.6+2801MG3 J221240+2759?ïø0¿KÁ?C²ÍäØò?O=çã:Â?C²ÍäØò?ïÑÆxÂ+?}åÏ6c[?wÿ6Óþ?}åÏ6c[?ïÏl±¦x?wíxGö?xI§DzO?wíxGö?ïjo˜ûJJ?x¾õáã?'²ÞÞèÆ?x¾õáã?ïÄ7ޤ̺?y0'ÅF:?}äÍåöô?y0'ÅF:?ᅢi3?¥nlã5Íu?(¡ZCž?¥nlã5Íu?óW"?Œý¥­…&?Œßƒ4‡®ü?Œý¥­…&?í"ÁÒ(»?žÿ¯l!Û?³YñpT­«?žÿ¯l!ÛAGN4FGL J2212.8+0647?êõtYe™ÀCfƒ#5.À9ÒÏr™zÀ;Ø£'@ßÄ@/1ÜF‡@m«w?¾fLæ¹Í?Ãx~‹ì@'pŽ@ÕO¨3æ?Ӝ=bá÷¿âS	AÈ!l¿ãܸ2¿êÊ©ÂÉn¿éö•žoû¿ïþ-͘¤§AGNfsrq1FGL J2212.9+0654TXS 2210+065?ïø\ÕæH?Oы	¹£§?OªŒ¸XAp?Oы	¹£§?ïÜ%
Íë?o­Wö¥¥?q÷m…w¢F?o­Wö¥¥?ïÈlC±@æ?uLr9ýSˆ?{ÉÞ9="·?uLr9ýSˆ?ï©;-†(¬?dè
³à?…±4¥Uí?dè
³à?ï©]†îÇ? &"§?ŸÊÔTI'? &"§?ï6끘Æá?›ÉЙÈ`?™"Æëð?›ÉЙÈ`?íŸÕ•?º"?¤àØI7ƒ?³SV.ó?¤àØI7ƒ?í® !1?–"éHiù?²Šþ÷ò^e?–"éHiùAGN4FGL J2212.9-2526?˖[îà•NÀKHßÞøH|À9Æ÷ê‡È·À<f1ØÀ @©þÁ'…@DAãÐ'?µ_ý–™4?ÀT5¡Íoµ@áDS@fý5uWÆ?ïeç}R;¿Èô 8Y¸®¿äövŸ´'¿âŸb2Ô¿éKòJ·¿ïÿõž}.)AGNfsrq3FGL J2213.1-2532PKS 2210-25?ïû̹£ò…?6ÄÐÿ2b?@Íñg9·?6ÄÐÿ2b?ïìíp;ž?e#"LX>J?cÁ'ùÖ?e#"LX>J?ïÈ+"W?z‹<{XŽ?{ê=´3(l?z‹<{XŽ?ïö;†œoj?@_F…?Sˆò'hûl?@_F…?ïêiZ»k?a±ÛîŸy?e–ú¾ÄÚ?a±ÛîŸy?ï¢÷!›Av?®ï'‰{¢?‡B7œŸ>'?®ï'‰{¢?ï:a'7¶?'Ø"¸*¿¡?˜³Û€s*?'Ø"¸*¿¡?ïêÈï%Dç?Vhº•›êÎ?e7VA-?Vhº•›êÎAGN4FGL J2213.5-4754¿é"ôTŒÀJƒ2a|ÚÀ;†¯²	ÓÀ<²§$œ—{@ ´-"¯¹?úèleƒè?Ð04:Å"ß?ÂîräÎ÷?ò"ÏÝù@'óƒðºé?ïû‹'™¿ìYÙ$Éã俵Ûc¾k`¿âc€4
¿ÃÇT}ZÉ¥¿æí¦a(9AGNbll3FGL J2213.6-4755SUMSS J221330-475426?ïþãߧ´©?Ö g­¤?!Â1%Sõ?Ö g­¤?ïõM7Hõ?YU'AZb?Ue'ÞÈûl?YU'AZb?ïê•o¾Sã?n¸Úo?ej±?n¸Úo?ïý5Üõ}µ?! þïvkÃ?6Qðcw@?! þïvkÃ?ïþcGD"Œ?(®· >?)ˍÅHNv?(®· >?ïØPSƒï?xx&Îê?s×Ö\jÔ}?xx&Îê?ïâ¦-Ú6u?tR͓*n…?mYÒÊʪ?tR͓*n…?ïø™]£c?C°Tø?Mš‰´ù?C°TøAGN4FGL J2213.9+5948c¿é¸a\€"i@½ZiÀ:ôÏJVÀ;N[`xæœ@É"
–ÜÑ@l¥³Û?еHŸ¸?ÀNL(Í~£?ö'SZ(@GMƒA?í#Ýàpm¦¿æ͕ŸŽü¿éÕÀ˜áä¿å|ßÿÚkF¿ä9AG`¿ïùÅôkwGAGNbcu1FGL J2214.5+5949TXS 2212+595?í½Lƒ³ £?Ð7 iÍ?²›äˆ¼c?Ð7 iÍ?ïτžÏ}E?}—²uåÓ?x=°ƒ£µ"?}—²uåÓ?ï©ðW§—ð?‡Pž½•®?…ƒê#Øsà?‡Pž½•®?︁cd"?d?-iÔÔ?ß§Cžî?d?-iÔÔ?ï'[O'ã?ªØä
J?i,««<?ªØä
J?î3h¿ËÌ?³E/y´.Ã?¬Î	rKu??³E/y´.Ã?íÒ*%²0?©w3Taa?±n®Ð¶±ð?©w3Taa?í=>tÛ?¤Þ=òÛ¨?·Æ$T‹,?¤Þ=òÛ¨8AGN4FGL J2215.4+0544?á×~4Ês<ÀCý—€º¥ƒÀ:¯¬kbOÀ<ióB'[@^´¸ƒê†@†ƒd£î‡?Ärj@:­¦?´Eyܺր?ðé›9¬Éø@ár¤P¿ï«.ýn€;?ïÌÄ¿77û¿èê~eᆿԑMjÙ¿çÂ[úҙ•¿ÈNÕ:¯~]AGNbcuNVSS J221513+054454?ïýwƒ³íò?&¨m3Æþ?4C⁌«ù?&¨m3Æþ?ïâ/ù™¬?o+?Á…tµ?mÐä…Ü?o+?Á…tµ?ï﬍Ů?Y]bY°T?`ìSGŸ)½?Y]bY°T?ïá­\D#›?RHêï;{p?nR£ç×d]?RHêï;{p?ïú¦½‹«?@€M—¾"?Eg´k|îT?@€M—¾"?ïgàÔ8u?›žá¾1ºž?"åxüQ[?›žá¾1ºž?ïå˜0ôû¦?r3v|—Ì?jgÎÉÚ!?r3v|—Ì?ïQе9³*?†ñÙÄõ?•ÅéWÌÁ?†ñÙÄõAGN4FGL J2215.4+6105¿®7Ðf_Z"@
ª:›À9æ†t"çŒÀ;edù~Ü@GK1¬ ]@øÍ ¯¢ð?ÌèæˆàŽÌ?Îü¿¿s@Õd¶býü@y-Å
5¹?îFÉ))?šg8ÚxBB¿çÄô'6ô‰¿æºÊ×)G!¿ï'>ˆPò¿ïíx:¤AAGNbcuNVSS J221507+610506?ïâ
™?¥{Gc90?®@Oä?¥{Gc90?皝¤"óß?ÆeÆm{ó?ÐÊĶöB?ÆeÆm{ó?íöv±Y¡(?š=3¦Æ^ç?°LJv|Ñ:?š=3¦Æ^ç?èœc /Ø,?£æíúT?͎q@ŸO?£æíúT?çNò¿$Ä?ÀÅMV?Ñb¶xø?ÀÅMV?ÅB¤àtŸd?Ç]:$¶e$?ê¯VÇâØ'?Ç]:$¶e$?ßyÊ˄'?º~ê§åGÿ?àCš=¶ø?º~ê§åGÿ?ǽB7ª^?¨Y¨'Å?ê9¯ri?¨Y¨'ÅMIXED4FGL J2216.8+3103?ïûw%Œ'±À5Cú*ÓéÀ:'S"¾À<6­•Ïà~@êûRò\@¼¾´ .?Ê\#—^ÖÐ?Ìvh&¯í?þrÉä»@ÅR¥>hq¿­QƒD1w
¿Ùè:œ3&ô¿èï^&üĿ拃ŒÚ¿ïýŒÙT›¿ðAGNfsrqS3 2214+30?︈@®=?€H€Ùû{?Ýþ`¶(¼?€H€Ùû{?ï¹5ws?Uâ	ÊÚ?²¢7£‰u?Uâ	ÊÚ?ïiĀçµË?…]£é™R?'ÇoÚr@©?…]£é™R?ïZ >RºÒ?sô™{+çZ?"»ø0;Ð?sô™{+çZ?îï­gàB?¡[ÔÍXU/?¡%6xì?¡[ÔÍXU/?îIÞKáf?²Ð­íc›0?«bAéž.?²Ð­íc›0?ìUßfh¥í?«Lë6?½Q̺И?«Lë6?ê÷A¥Z?¦¤Ì@w?Ä"ùkޗÈ?¦¤Ì@wAGN4FGL J2216.9+2421¿ÐÒZ?ÜÀ:r¥'ÛçóÀ9†B"ÏÞÀ<*4žm>@oâ~9ì¶@é©¿Š¯?²˜;J®Ïâ?¬uüº?ø·…Ýúòz@
°ÕöA:¿Ò}ÆUˏ¿á>Ÿ&Kn¿å–¢='¿ãh4çÌ-¿ãîª!üÿð¿ì…ΫÊÆAGNbll3FGL J2217.0+2421B2 2214+24B?ïþs"]€Ë?
àÆËø?(ƶ &ä–?
àÆËø?ïîFè$u?fk82ûm³?ao¸ã¡{–?fk82ûm³?ïöì­µ&à?>W:+ÑfN?R&¤Vyoì?>W:+ÑfN?ïùÒ{_?364†?H·Ñ¥^Gü?364†?ïüéɚ$?2€C	Ž1‹?8·çÈÍt?2€C	Ž1‹?ï¥ËõJ?ši`(Ð&ö?†ÁØ%f?ši`(Ð&ö?ïòXnoä?g@öLxš?[O#ë*Ÿ?g@öLxš?ïíƒ: |?Q‰†Ü:™}?b|ŧ*X?Q‰†Ü:™}AGN4FGL J2218.6+1941?Ù<®É£ïÖÀ>P;€AÀ:ß!5Ú­`À<L½}®'@˜o¢û@V	™Üµx?Î
	}Ø
?¶$ø¡«¥¥?âÙ`>.8ø@´4¥y!¿Íg³BW¿Û•=׿és¹jð8ã¿ám —d¶¿ïÿÚpú>?æÓó! 8ÅAGNbcuGALEXASC J221854.64+193841.6?ïü뜁ç‡?2;ŒÏN-?8£jp&{?2;ŒÏN-?ïéxøö\¤?h§ô÷Fq¡?f‡&€?h§ô÷Fq¡?ïÑÖ¶Ilt?qè3'T?w¤Óº¡Ú?qè3'T?ïö"è¡Ø?=Á';´ô?RÖ/†‡As?=Á';´ô?ïü,•yT?> ©£Ý?>›Ué»úÓ?> ©£Ý?ïßŠV«?"(Ríªì?Œˆɍ?"(Ríªì?ï[\5ú¨?ˆâÂÛÆà†?ˆ©)?Æ?ˆâÂÛÆà†?גּ¡0?vý5þ9'?"ÓW³ùŸÇ?vý5þ9'AGN4FGL J2219.2+1806¿ãr"'¿RÀ?¢i'ÄÀ8þÏ;<1À;×Q!ZÛ@¢ª‰Uÿ'@l@šú©?©¦"Ô¸Ôr?µh¯‰â@
¾cb¥ç†@"Êb9[¿Î"¤)•z¦¿Ýˬ;\Í`¿ãü& ûù
¿ã@/€ Kпè|·áƒ=7¿ìbíç$AGNfsrq3FGL J2219.2+1806MG1 J221916+1806?ïþ	e‹l?$¹
֔°m?/o<ßës½?$¹
֔°m?ïëæ¶?gO•Ÿ?dIîÜ¥1?gO•Ÿ?ïáд°BË?ošZæšh?n/K;O?ošZæšh?ïÿ¹zßf>òèNÌ-&?¡'¸p/>òèNÌ-&?ïû4˜È?FþBó+?C/¥]gÒ1?FþBó+?ï£p*"2?"l…ý?Y?‡#õhýc{?"l…ý?Y?ïµuIÐzú?"b³Ö*`?'¢­|k±?"b³Ö*`?ïÿ"TlO?xQÌæëè?*ï 5/$?xQÌæëèAGN4FGL J2219.2-0342¿è®ËÆx°ýÀGfá`؇ìÀ9Ê©Hš¤À<*yØ32\@蹃ÄÆ@ôɅðoi?»Ë"?À. ý;)¢?ü6öl‡š@íèQ¸"k¿ÏX"¿åޗ¿æ·û"p=¿è§:¬Î*¿éÉc@—ë¿ë³@S'D¿íý}¿HÌAGNfsrqPKS 2216-03?ïÈn;ÐnK?´\žÅ‹7?{Èáþ[¾Ù?´\žÅ‹7?ïícÃHê?e
*ΞRÎ?báœeòeG?e
*ΞRÎ?ïÍUݤƒ?~µvcCz3?yÕ®^¡?~µvcCz3?ïý™%€m#?!~®ZÚÊ?36ӎ£j€?!~®ZÚÊ?ïûbü›éÍ?CWêK%Ï?Bt)ºŒò?CWêK%Ï?ï£1­÷õp?ŒôeÇú?‡3""0°?ŒôeÇú?ï"9'Ê}?Œ–(ftª×?Šñ›‡\4œ?Œ–(ftª×?ï÷&3ć?CpßÐß?Q³™ÁýÑÖ?CpßÐßAGN4FGL J2220.5+2813?Úg»—žGÀ7ÝÀµgÀ:Dmî$À<z8Cƒã@ ÷X¼…?ÿ
ä)à¤?ÂÁòh½®¢?¥Ø£š¤\?ã¹
"BË?þ'ÒÐÇÙ?ïú{üР—¿è¬Ôÿ÷«¿ßd­ÿ'+¿¿ÜÆOo©Ü¿Øå$ýd¿æÄç=AGNbll3FGL J2220.3+2812RX J2220.4+2814?ïü°òž·?0C
Ù%'Š?:xo|….?0C
Ù%'Š?ïêåºb®?kütÜ&+@?eE³ãѲ?kütÜ&+@?ïó^K\AA?PŸ;T¡æB?YChêÃ?PŸ;T¡æB?ïâHÉ꼙?Oú¦Á³@?m·6 B&«?Oú¦Á³@?ï÷¨o§ý?IÜ0lŠÍ?P¯ û–5?IÜ0lŠÍ?綠þA©?'š‡î/û?†þ|ÿùÙ?'š‡î/û?ïöÊǯà?\Ûï&Zœ?RkÌ`" ?\Ûï&Zœ?ï'AvK?s©b±oò?‹x½]?s©b±oòAGN4FGL J2221.5-5225?ß8çJ°ÀJ1	á*QãÀ9vvü¶ŸdÀ;ñžbeP@üDËaé?ù½R;66ô?°«¶ý'¢1?ºˆ©t
n@‹"ÞQZ@Öjˆ	#j?Ö\_ý@²ù?ËÙÂ~•1U¿Ó¹Ššù*¿Ó«<äâÃ.¿Þ Ý%	¤Ä¿ßÝD>HeAGNbll3FGL J2221.6-5225PMN J2221-5224?ïýŏŽ?2íô!hó?7ÑÒYàø?2íô!hó?ïôØJ•‹©?WÂì®$z?VOkBÜ-?WÂì®$z?ïÛ&Œæó?w<w¨w?rlþ±MvË?w<w¨w?ïø¬¸ôíl?4Fl%G¿Æ?MMÿe¬?4Fl%G¿Æ?ïüZXˆy®?8‰~nŒÊ?=-<Óy4q?8‰~nŒÊ?ïÓõ7FŠ ?} Ó|PH?vdsh¹?} Ó|PH?ïÜXœŠuö?}}Å1M?qÓ±Ïb¬²?}}Å1M?ïëϵ›"?S³3œ+C¡?d0J£¤ÎÄ?S³3œ+C¡AGN4FGL J2221.9-3504¿ïÁ£n.±ÄÀLžÁ~ºñÀ:ÆùáØ͌À<§¾Ê«Š]@û±r(f|@}õÏ$•á?ÉìtÝÍ{?Î3†V¤?÷E¶ù%ñ+@­ÇÜMj?ïþ[Ï߿⿛L4¿çîYyîÙg¿ìîiÀ
 пøÌ?îÛ@Î&i AGNfsrq3FGL J2222.3-3500NVSS J222227-350942?ïÙü)u‰?¨0^w²ÿ?së+Î`.?¨0^w²ÿ?ïí´Tõ"†?fÐÑ/Í]?bK«.'iÖ?fÐÑ/Í]?ï1'æ£?"4O¬ ì?™Í¯ÙsŸ?"4O¬ ì?ïüT5¨"?,'€@e?=^X†iª?,'€@e?ïý¡¹M¾û?DˆN<Å7Û?2ò5x¾>?DˆN<Å7Û?ïi+µ?"þ·1ƒPo?ڎ†Š?"þ·1ƒPo?ïnnó}¼?•ÿqLÞ?r2!H?•ÿqLÞ?ïîhÝ}ãÊ?T,ÞâÑT?a—"–¹ÝŠ?T,ÞâÑTAGN4FGL J2222.8+1209?ï¾îÕW­2ÀBWìÝ
Œ°À:c5*"8	À<8wškP±@¤ÔpZ0"@/MzÝð?ǜ
b.žN?Ł柆Ã?ü!¦ä÷·@T?b¿â½/k'–G¿áÎ耇yÜ¿åƒ) b`¿âя–n¿ïõ´yÒª¿ï}lÝxì{AGNbcuTXS 2220+119?ïø|2Öl?CÃ¥¼Hï?N4'Q"L?CÃ¥¼Hï?ïçEÏˍe?m!T|ñ¥š?hº/þس?m!T|ñ¥š?ïØ©C§z?pp
×?s«^v+£?pp
×?ïïüÎXyO?E'qó2Ãi?`1¶¤øã?E'qó2Ãi?ïî`€üÈF?`ŠCmšN?aŸ~àÛ¢~?`ŠCmšN?ï"g¸˜YË?'§bœ?‹&Ϛ¹S?'§bœ?ï•ùD,³E?ˆÁrÈìºË?Š®íóöÎ?ˆÁrÈìºË?ï³tì2?rŸ¼g·?ƒ"Ä턤&?rŸ¼g·AGN4FGL J2223.0+6746¿íÔ\B@!©Õ<ÝÖàÀ:~?Àà/€À;Ú@@aïß@dða|qÁ@K³ŸÕý?ÊÜøHр?½û
wÓ N?ò_V§¬Ô?ö"hëPñ_?ïî}†¸–¿ç6geiç$¿åý·³àm¿å  †Þ+¿ð?ïÿÿ)@k*AGNbcuTXS 2221+675?ïÖA%·—?q®³%Ú?tß1Kx°?q®³%Ú?îí:	U*?©9]0íµ?¡,_h(h?©9]0íµ?îöT</^?–(Xêù? š¼Cè?–(Xêù?öMŠÞ?ŒJÅñÈL
?¥öН»?ŒJÅñÈL
?ïG¦èK·?šì¢L"?—<iÕÁ?šì¢L"?ä!¼?Ò¹žÐB֝?×½ñÁè‡?Ò¹žÐB֝?íÀÇ}O?¦\ꒊ¥™?´ùç"l?¦\ꒊ¥™?ã3²P:?¹e$Dád?̛ٙ_Ӌ?¹e$DádAGN4FGL J2223.3+0102¿çW1õÆk4ÀFMa€M˜9À;>Õ'åÀ<‹wI¹L@ Äkq=/?ü›Þ'׶5?Ñb
-€l?¿¶«G—?ñÞâ^.‰€@é£È¸?çÃ_›q
.¿çXÛch…%¿ãØMꣿÇÍ×0¨ê¿Ý·R<7馿Þ4hݏÖAGNbll3FGL J2223.3+0103SDSS J222329.56+010226.6?ïÿ"é?SYø	?¿Â¶²S?SYø	?ïí=ø:?dʚS?büÂ6Ö?dʚS?ïøßçÔŸ?:¨\h÷£?L€a´H?:¨\h÷£?ï÷¨˜E?3­µ}A–¾?P®ÎoDGŒ?3­µ}A–¾?ïþëwª'ÿ?Qý€'«Â?!H"ΐW5?Qý€'«Â?ï›çš-"6?Ž~Pºmÿ¬?‰m»ú?Ž~Pºmÿ¬?ïöX<?»?^§ýöÁ?SOÅXÅÚ?^§ýöÁ?ïá0*%~¦?]~oì©æ^?nÏÕÒBJ-?]~oì©æ^AGN4FGL J2223.4+5814¿æhO(v®?軈!!7ÞÀ9ƒÝòŽþ5À;'éÃ}˜²@ºµ ¶Cs@Ù¶3kg?ÌÜ9|Mƒl?Õâ‹ûÌ>²@é!S6ß?éðŽîoß·?ïûøi2Ɂ¿ãç—¾Vè¿çðSà&ñ±¿ï6©	y&¿ð?ðAGNbcuSSTSL2 J222330.04+581350.9?î«ý'C?ÄÍ¡€e7Š?®å@*_Ø?ÄÍ¡€e7Š?×JM\U…?Í é}?äZÙpQÕ=?Í é}?ë&Òlžä²?§šjþ:Rî?Ãd¶M"m8?§šjþ:Rî?Ùqô|ǯ_?¶¸27w~?ãGÁœ(P?¶¸27w~?ï'»ö»?ƒ®=9?‹xQµX?ƒ®=9?›zLºRR±?¤åñlµ8?ï$-š®û?¤åñlµ8?â‡Z¡iÐ?¶ÀÉS(n?ÚñÿJ½,`?¶ÀÉS(n?'ºt;®Z[?…åä]k?ïr,^>

?…åä]kMIXED4FGL J2224.0-1127?ï!h€ÀJ­>'À;X"üS£À<m
Ø/×^@¹¡"I¦<?ýœ>	P
Ú?Ô38üö¶*?ØÀyJ]@4…]¢r†@Fg˜jš¿ê6ñL¿ëk»À5Ö¿Ò\rœª›¿Û×£TY¿é4ց+Ž¤¿ïV›LøWAGNbll3FGL J2224.6-1122PKS 2221-116?ïñ¦^V«?Z'u÷r¤£?\³Cœáok?Z'u÷r¤£?ïæu"w°?kwM50B!?iîŠS¬Ø—?kwM50B!?ïq¥‡—:?ˆÓTÀ?'ËOüp°?ˆÓTÀ?ïؔB©À?ZU'ÄèC?sµõq9Ô?ZU'ÄèC?ï·VÀúÂ?ƒn/«Ëp?'*Oü@ÿŒ?ƒn/«Ëp?ï"\Pbîã?Ì®Ûr?Žèëî#N?Ì®Ûr?îŸéi7?™®¦'¼ºã?¦oEüò+?™®¦'¼ºã?ïHr_˜?†ªRÞÑ‹?–ýѵ;vÿ?†ªRÞÑ‹AGN4FGL J2224.3+7737¿àÁ¡ÕŸ¦›@1€¾×@ÄÀ:yôºQ À<Ó'¹¬@*CÜ΢@ˆE~R?Øb«{™Sy?ÜÓ¸#rué@ÊÊ¡yaì?ü¨pÄä &?â{à­Tb¿áʁ=­4¬¿é1G ¨"¿íè?÷g¿ãŽYÊv±¿ïÿÿ>¹úAGNbcuNVSS J222721+773319?ï™üO"³s?šÔEÊõ?‰€ì(ѓ-?šÔEÊõ?îTáªïE?±Ø¦Ôþe?ª±åS¢«?±Ø¦Ôþe?î	יPì?º>[®$?¯nB…
D?º>[®$?î¥ù>Dß?"ÊÐá=ú?¥¯ i‡ý?"ÊÐá=ú?ïJB)¬\ü?¡Û$¤0=¹?–·ºÍãü~?¡Û$¤0=¹?áXlææ²?ÑáWáñÖ?ÝO&22›ø?ÑáWáñÖ?èŠéåƒÊ?¸µ˜<r-6?Í×ÐXið×?¸µ˜<r-6?å\pe»?º—y-éGW?ÕûG4‰Ü?º—y-éGWAGN4FGL J2224.5+0353?èÃðÁYãÀEriƒQX¸À;`P‹2ΉÀ<ž>xá"@ ËÕ§½?ýÞeæä¦?Ð#$< DY?Á>ڛÂhÆ?ó&eYöì[@'Ãfœ—%¿í²æ§ieõ¿îEÊ¿×Eø?ïÿë""i·¿æ
Yº†y+¿Ô7ü:ù{,¿â¯má"ê¶AGNbcu3FGL J2224.4+03511RXS J222426.5+035445?ïÿBñX1?
n	)ƒ?¡åQu±?
n	)ƒ?ï럳Æ?jµ•ÆŸ?d`Mß¾?jµ•ÆŸ?ïïáÑZ"æ?jψah?`.çc™à?jψah?ï÷é¢×}?=̹S‹©Õ?P,»®
Z"?=̹S‹©Õ?ïþ.i0?)‡Ä?-8GÃ?)‡Ä?ï¥*4Ãs?só-8ç5?†µrÈ\k4?só-8ç5?ïï'â<Ã?höxÑó?`ñm+¬÷?höxÑó?ïçóƒ¬?al5A-,k?hî°Žÿ?al5A-,kAGN4FGL J2225.5-1114?íº´'!ëÀJ"Ĥ	_$À:¨ÝÛ
À<OÐîš|î@ÌÁën ?÷@]Øù*ú?á°Þ1Î?â5~†mÃ@ïƒ9@ØS"¥å¿ï;Wú'ص?ïí%HzÿåŸ/ۏÞ/¿Ük®Œp¿ïÿÿ" 5•?ïæ0¡¢AGNbll3FGL J2224.6-1122PKS 2223-114?ïìVâ²3¼?…ÐÁÂæ@¨?c©:Žt_?…ÐÁÂæ@¨?ïåÄ^$‰³?w¶Ð}°«Á?j;¡¡¼Ü÷?w¶Ð}°«Á?î04-?œu†¸íý?¬÷,ºÑ«7?œu†¸íý?ïç1ÏšÕ?W£U"zâø?hÎ~Kâ
?W£U"zâø?ïãwuFAó?{U©çÜÓï?lˆŠœáU¦?{U©çÜÓï?ï€Ýò¨ÃG?ìÉï=?Èƒ\®f6?ìÉï=?îUB
Î?ž1@DÍÌ?ª®ïÞs"?ž1@DÍÌ?離(ˆ	y?ƒƒÞŒ‰Û÷?†uӮͺ?ƒƒÞŒ‰Û÷AGN4FGL J2225.6+2120?®ÀÓaÿ^À>ó^1
¿À:\‰mÒkÀ<.2$?zi@Œ9j.òÝ@4ä†&ö?ŝZ³Ê?ÑöJ>ès@"éèwM@	¸§áÛÒ¤¿Õê£	"¾¿ç˜¨"HK¿é¾Ðà­ªH¿îš¿^z4¿ïò$_°¿¦?ïw:ÿ°NèAGNfsrqPKS 2223+21?ïûz|ÈÓn?C÷/¨?BëŠ1–?C÷/¨?ï⁽.õ?r'y&õr?m~B½Í%?r'y&õr?ï'fZZ
?ë‹:q?‹¦iX*°Ð?ë‹:q?ïâˆÁA®?YÍdñ ?mw>DŽB(?YÍdñ ?ïùs£³l?N€ÅQÝı?J1pb®?N€ÅQÝı?ï8
¡íêÃ?¤pãЛú¢?˜þKÂB§'?¤pãЛú¢?îÿ³nN^ª?"¨B0òŒ? É†`a?"¨B0òŒ?î‡äp,Ó?™Žµ;u?§¸ü[;Ø?™Žµ;uAGN4FGL J2225.7-0457¿çu!ÓörõÀHjœýÒ(VÀ9θ_WÀ<
¥T¸¾ù@š"ÀC§u@úÑÂÕÓ?«Fg~¥ˆ¡?´QVßµ²ª@—9~¦Ï@¦Mhky¿ÃöXak¿áâÈa®Û¿æÜrÒ¨"¿äØ`^'i¿êTCƒãNï¿ïÿÊñ*z'AGNfsrq3FGL J2225.8-04543C 446?ïü6bMä?P^'/Sž??MWx	?P^'/Sž?ïï9X]±ƒ?dáxïj²'?`Ƨšl¤?dáxïj²'?ïÅA–ßf>?'Wj	Š?}_4 Ë?'Wj	Š?ïþ¨Ö½*\?1qÚüâ?%r˜N]f?1qÚüâ?ïù}ˆ¨ï?Fórãì?J	Ýe'¢]?Fórãì?ï—GÖó5?•Öcõ(þª?Š.
M†Ï?•Öcõ(þª?ï™ÔÑÂÄ¥?ŠâÐÆá¹4?‰ŠË™ª³?ŠâÐÆá¹4?ïý}!qrg?+A‰™†?4õ¦Õ¹?+A‰™†AGN4FGL J2226.5+6901c¿êÇЈ2õ@#mfŒ&À;L‰~™cÀ<FdÆ@"퉰ÃW?®ìc.è:?æÚU웟-?ïþÖ¿ê¼!@¤Œ;ã@¾i¼²"?è0Ì ?ïò솦wοØö™NðþÛ¿â?Ö¿¿É?´ß´°÷.¿ç|<[Ðá/AGNbcuNVSS J222625+690207?ïÚÍk7?tÿ¤w…?rö{iìM?tÿ¤w…?ïßprÁÆ??=rW?pGÆüÜµ??=rW?îv5ΐh»?Ÿ tøLá?¨œ£iN?Ÿ tøLá?ïØÙ½öñ?gàA'viN?s" ð™½L?gàA'viN?ïfž«¸f?'Ëxš©Ã?Œ¦XN2®w?'Ëxš©Ã?ïO£Q?¡:½"õŸ?–‹¡ä_É?¡:½"õŸ?î–â(Ã\z?šL¿Ô?¦'ÝsÊ8Y?šL¿Ô?ïßkl×æÿ?võ'Pm«?pJI®)ˆŒ?võ'Pm« AGN4FGL J2226.6+0210¿Ø@àÏ|ï.ÀF;€Ü3rÀ;Y.yÖÀ<…¦Ž@!¸IƯc?ûÓµõó?Ì^ív:™Ú?¶&	>˜7?ì%vå@ú5ÏÅ¥'¿ìÉW,6À¿ïÿóÖ&ã?ïÿꁺ¿à>"7Z	¿à	bŸ‡oK¿»'®îÀhAGNbcu2MASS J22263636+0210373?ïÿv26^?{§q½g?9Àýpws?{§q½g?ïìzÃ{Ñn?g¦Z'ˆ±R?c…<Gµr|?g¦Z'ˆ±R?ïø¥é34á?@º4ÑÍà?Mh\ßHÆ?@º4ÑÍà?ïú˜|äG?5©OˆrïW?EžÅÕ>?5©OˆrïW?ïÿ•‡Éã?mŒÞ£?
¿.»&ÈQ?mŒÞ£?ïœM`…ü¯?–}l‹p@m?ˆì§Þ€ÔQ?–}l‹p@m?ïøôn¸€¡?ZqxÙª?L.Di+p?ZqxÙª?ïó¥¢¢'ù?Q¢§!Óøƒ?X´ºœ~Ü?Q¢§!ÓøƒAGN4FGL J2226.8+0051¿ï®£Y5ü;ÀF°CécÜÀ:2lÙG."À;á/Ø4ßÜ@§¶¶@F€d?ÃßÉi@
‡?Îz°m¸@Œ:䜸@×æ\ÀË7?ïÈzW´ò»¿ÀÐâC5à¿éaJÓbé¿ç޻♽¬¿ïÿŸR@>´?ê1þ –
AGNfsrqPKS B2224+006?ï漐G>?gSÃY°Y?iCoŠE'?gSÃY°Y?ïªà,6P?"{9";ßê?…GôüºÒÚ?"{9";ßê?ï}¤Â'éd?"U-ͱ-?Kg¹Kz?"U-ͱ-?ïb2¡W?qç{o«•?Œ§{vÇFK?qç{o«•?íÛ²ê­]?³¿GÙÝ>?±"oA†|?³¿GÙÝ>?ëÄ_Q¸ô?ÆeÅNÀ?À/¥?ÆeÅNÀ?ë;ŸÀûs?®d‡1?Ɲ?Àüâ5?®d‡1?Ɲ?ëð¹ø?¬8»
?ÃÀ=—±?¬8»
AGN4FGL J2227.9-3031?çˆv‡ÅÀMAð€0<À;n4˹§VÀ<ØYí²¢@ ò0´}Ì?ÿlº=~?ÊYÐ@tº<?i6+»W?¡±‹OÈâ@®©ÌĿ¯ÂÐË?èéÅ+Û¿¿Ö@£[å.¿èºÿƒ¿ÄõÊ\…!¿ÚÄ^Ô¡­dAGNrdg1FGL J2227.7-3036PKS 2225-308?ïþž=d±Ó?!½L‡.;^?&%¤¿Ý?!½L‡.;^?ïî]"ÅÒ³?fò³¹oë¨?a¢ÝA…b?fò³¹oë¨?ïÜ\öܧ?r~nIц£?qѱÏ|m?r~nIц£?ïþÁzøÞg?ºbsíå?#èM7DZm?ºbsíå?ïþ9–ϏË?,HšÁin½?,fvYï?,HšÁin½?½ò$±?Ió"æ?‰Ð'5Cš?Ió"æ?ïÒª™?^xJÝP€?~·ò'(Ó©?^xJÝP€?ïû˜/?9aEé»êU?AŸ!Þü$?9aEé»êUAGN4FGL J2227.9+0036¿ï©±ŸtÏáÀFÞùü°À'À9®GE8ï5À;Í´ÚgÀ@B89,qx?ÿNlªMF?¶
ï×¾ÃJ?ÀB}þÞlÝ@	†)vò@&ם`Mž?ï–<¢¤@¿Û¥oÛÛ£¿Ù²¬…Y›¨¿ÙÕyäÈl¿çr4/²u3¿Ýí¾Ÿb†]AGNbll3FGL J2227.8+0040PMN J2227+0037?ïû‰†¯®?;©:úߞF?AÙæQUšÎ?;©:úߞF?ïÒñû
/œ?vݺÊ.?v‡q)"
?vݺÊ.?ïéP˜&†?aÁsÞåI?fí¯?þ´?aÁsÞåI?ï€A®À?lå¢0ióÅ?ï¾—¿t¬?lå¢0ióÅ?ïÚ׎5§?rÍ'*†O\?r"8컖£?rÍ'*†O\?ï‰ßDã?¡z+40;?ŽÄ‡Ç ?¡z+40;?ïsŸujÌ?k'ÒS^?'Œ\#
?k'ÒS^?íxpÉ?™D[îvk?³|?í[º?™D[îvkAGN4FGL J2228.0-4155?¶üÿÿÛìÀL¤ÿiKÀ;Óúú݁PÀ<ö[ªJÁÅ@!ø-ƒpã?ü'/"R	¸?Ð`û£$ð?´ñZuÂNï?êð¾'d@fRðÜ¿ïÝÜ>¯¾?Þ?»Ø?ïʵe§ú…¿çÒ¿?›vi¿Ës˜=£úq¿ÏKi W£ÖAGNbcuRBS 1864?ïÿªÕ¬y?ÃV Í^=?J'¥±?ÃV Í^=?ïö˜×k?V¬AÓé-w?RÏψÙJç?V¬AÓé-w?ïÖ¸¦z'¹?zìÛÊé`=?t£¬ÏJ»C?zìÛÊé`=?ïþ;2—=/? ¢­¨¤?,LÒéý9¶? ¢­¨¤?ïÿÆz*ñú?4ûWн>üÂÍùu€?4ûWн?ï×%`Œ²«?^Ö°Áuv?tmOؓ&#?^Ö°Áuv?ïÚkÚ!Q½?zK%j[]?rÊQi?zK%j[]?ïûϤmˆ?;óòÂ1Ê?@ÁmÍ ðé?;óòÂ1ÊAGN4FGL J2228.5+2211¿íMÍÈl¸2À=ÊøzЀ¶À:v×ÁóT÷À<Q¬Ô	1@ë9¸2‹î@A©¸ËŽ?ƪ×Y˜¢¤?Ãõµ¹µÃÇ?ûPÔ´!Û?ü«H%2¿p?ïô›?¥¿Ô6«ÃgÉ=¿ÛRDËáë¿éâd®ÖAÁ¿ä‹*5]¯Þ¿ðAGNbcu87GB 222614.9+215540?ïê2–Þ±Ú?`Œè&Ï?eÍifUk?`Œè&Ï?ïAÎ×i?–Ž‹YÌ
k?¯Œ?Öê?–Ž‹YÌ
k?ïŸ2ׇª?ƒT:îâ{?ˆ3Ja¥v?ƒT:îâ{?î¿
c:ˆ?'ž_O¾}­?¤)Èä%}?'ž_O¾}­?ï""¦™?˜TÈ'xIP?›­‹$GT?˜TÈ'xIP?ì<Mÿù[1?Áיum¦ˆ?¾5&u?Áיum¦ˆ?î v(êôš?¢;Ë	£~?­ør,a?¢;Ë	£~?èñ!åqÎ?«í;~c?Ì9¿xj8È?«í;~cAGN4FGL J2228.6-1636?äå–È·qúÀK±#öM¾À:m›¨g'¶À<xÐÜüŹ@¿Î´-™–@?'yꧩ?¾âÊ: bK?™l#"¯¤ô?ܶe§"ê@²¯ï;¿ë¬k˜ÕN|?³'«hÎös¿Û†Iû̔™¿áðk֙տãȓíˆ.7¿ÚÖ Ř%AGNbll3FGL J2228.5-16362MASS J22283018-1636432?ïþËFºÏ?ÂPøáú?'ãIÍ dÍ?ÂPøáú?ïï\¹`Ö§?b~μ
Á?`£Fq΁\?b~μ
Á?ïñ
Iû²Ð?aHSRÈ?]ål!WÐ?aHSRÈ?ïþ½¬º±?H‰+:S¶?$%A'»Ê?H‰+:S¶?ïý]«×´²?-ù£À®©Û?5¢i¸¾?-ù£À®©Û?¬MÑD?ŽHÓ?‡X"ì‹®õ?ŽHÓ?ïñžm5Yö?fSêÓêîŒ?\Ã%ÆÆrõ?fSêÓêîŒ?ïýn¾'9ß?)[¦wµåN?4ŠF'J?)[¦wµåNAGN4FGL J2229.1+2254¿ïPdô÷8[À=M5e<š»À;€€ÃàÀ<ž£;M@ ôáÊà¹i?ýá©»Þh?Ép£×
=q?¢%¹øߥB?Ø:€›k?ö¢<þ?ïü±a6{½¿ã9 Š¤‰¿è»ÞÓ_Ž¿Ð"L€a9V¿áÙ|"MÀ¿Å\Ùê¦ÒAGNbll3FGL J2229.1+2255NVSS J222913+225511?ïý«±–‡ä?0(]&¶}?2¢töÎ-?0(]&¶}?ïÜÃÑë3"?{‡Î"ÌœÀ?qž,iÑ?{‡Î"ÌœÀ?ïåqËc/?r&˜'?jŽ4à)Dv?r&˜'?ïÐ\Ç´½•?[ŠrQ"–£?wќ6ÏAi?[ŠrQ"–£?ïþ_­ÿF?/õ¶p¡c?*"2àÀ?/õ¶p¡c?ïebþ°}>?˜q
IÔ:?"S # ;?˜q
IÔ:?ïèUª_E?tótÑk?gªUy
Bî?tótÑk?ï3>Wì?ŠŸIOâé?Ÿ˜:EŒ?ŠŸIOâéAGN4FGL J2229.2-6911?ÞÖ[8WVËÀE	 :2+À:–(òÀ<~•rÃkû@ÊIÞEp"@_þmXÉ?¼L^}cØí¿©"¯#æÜe?ì!$þ<0ˆ@æ)ë
û\¿á¸Dêë›Å¿ãB;䳿æ§Êêt}€¿å'Paí/ï¿ê÷¢cl·¿ïÿ¦¶tFAGNbcuPKS 2225-694?ïø+ü™Ta?G˜>|Ûa?OP
?lo?G˜>|Ûa?ïô¬`NR?_ëæþ‡F?Wú§§l;?_ëæþ‡F?ïàÚùéÄ?jJ·tþ)?o%Õ£QQ?jJ·tþ)?ïø¡*É?6ðu³h@?Oõxù~ùè?6ðu³h@?ïæʹ;c?c[Àˆ'XR?i5FµÓUb?c[Àˆ'XR?ïÊÏÒÄ;6?…üwʹc?z˜¾.¸ž?…üwʹc?ïÁçíÿ;N?&NÅ@´?ï4M1?&NÅ@´?ï¿#®}MÖ?r&"÷:§x?€7e$~?r&"÷:§xAGN4FGL J2229.7-0832?ÐB/*÷
ÊÀIÚÃ.¾YÀ7㸫­˜TÀ;¸<ù…'@6r$àŠ@ÉWòÓÈ?•ŽšPèj?¹^¸`óϊ@þU@ÓfI`I¿ËU+«u+¿äœ.܌¿è]º|h0¿è½¶ÿÛíÒ¿ìÀ©s+pÇ¿ëêM`ÛâêAGNFSRQ3FGL J2229.7-0833PKS 2227-08?ïõr¤Ï?`3\Õ?Kh?Uޚäú?`3\Õ?Kh?ïá°Þüò|?vCýøí%Ù?nO þíü0?vCýøí%Ù?ïg›±»"-?'s.I4>…?"‰ÍµM?'s.I4>…?ïú>MK?ø?9SÚ¹¤w³?GÊbÙ­§?9SÚ¹¤w³?ïú9¨÷Ë?D§¢X[?G_™jÁê?D§¢X[?ïZ	"Ê:Ý?¨°ÇzÖÊw?"¾ÏeÖW?¨°ÇzÖÊw?ï'TíSf@?ØÖē?‹jħ¶Ô?ØÖē?ïå¶,C?bC¿¯ò8O?jIÓáþˆ?bC¿¯ò8OAGN4FGL J2230.9-7815¿î®×"ûÀB="V!uÀ9ü›A9†4À<NB€Æ@$y&5@*t:dÜ?¸LêijÓ? §½sñó?ääýp-º@
›™pÿÇv?Ú¾..½¿ã²xÞ8/¿âhrzpßf¿åã¡$¨Uõ¿àyâš'¿ïÿ¶cÔ»¯AGNbcu3FGL J2230.5-7817PKS 2225-785?ïýžý9YÆ?$¯E°"Ú?3ü4ÄÁ?$¯E°"Ú?ïö'¾3µ?W@A']A?RÜzÍÐ$À?W@A']A?ïïê4ÖeA?cTûÀ
]°?`Ë_o~?cTûÀ
]°?ïý¼>	P?r`Ä­é?27=µF?r`Ä­é?ïûA‹ª\y?8‡D.%ñ/?BùÐ^¹?8‡D.%ñ/?ïÜC¸;›7?~#
T@kÏ?qÞ#͔¼É?~#
T@kÏ?ïèŸ+²hü?tW².<¶?g`Ô0ºL3?tW².<¶?ïùfðhÍ
?=ÍÉWÃÅ?Jd>ä•õ"?=ÍÉWÃÅAGN4FGL J2231.0-4416?íîÞr;±²ÀL5'Ì÷À9ÓÖxG9zÀ<†óEšN@tu%Çe@8TÛ#§¥?±vp_8Ÿ¯?¨œêB9Lj?ðxë¤(hÕ@,(¡3ìÂ?ªÛk¡
×.¿â}5´Âë¿ç "¦£m¿æðÀ'+ç¿ä$?	ˆ?¿áüâ©­ãÓAGNfsrq3FGL J2230.6-4419PKS 2227-445?ïÿQý_?ڀbEV?Ç°Åt`É?ڀbEV?ïõÿ=¸GZ?YÇl£/Ý ?T"¢¯"?YÇl£/Ý ?ïð!¯8x~?`5
³S?_¼¡Ëˆ$_?`5
³S?ïÿç1ÝÑ>ÞäÒtݼ>èæÌÐi®ƒ>ÞäÒtݼ?ïÿºÃ¾cÜ>ü÷W3_Ũ?O|ä¬>ü÷W3_Ũ?ï݀Še/k?tbP `?q?º¼:>¦?tbP `?ïç5›î2£?pÀ4 Šr?hÊdHÇž?pÀ4 Šr?ïÿÓðáÉ>ð°ƒ{w¶>öŽa_y>ð°ƒ{w¶AGN4FGL J2232.3+6246?âa«'¾¯@G"#ρÀ9¥s¶±•À;M`ÈW@b$uÖÿ@Q*Dw(V?ËE$wX§?ÅÍ£À#@w]š
_?ü…ktm:@?ïÿôa¼2¡¿ÚlUÿø¿è#†b/J¿åha}ÉY{¿ïüG¿e ?ï'[>ê÷ZAGNbcu8C 2230+625?ï´5§µCÍ?"]¯3°?'ò–?pÖ?"]¯3°?ì¼	VH"¢?»"öЈç?ºµM»Zñ?»"öЈç?îEjÀ"-š?™ZŒ?HRE?«©Sô9qh?™ZŒ?HRE?ëÃÝNòxÐ?¢ÂöðmØú?ÀðŠÄ6¿?¢ÂöðmØú?îº;ÙÂK?¦cüýÊv?¤^üEÓwK?¦cüýÊv?Ðå,5yDÌ?Ñi'"¦Ÿ?çiåC]š?Ñi'"¦Ÿ?å|ôeÿ•?·{"}ûë?Õ4ÂÖ?·{"}ûë?ÍÉ…¶ì?µLzh¥%¬?荾޼RE?µLzh¥%¬MIXED4FGL J2232.6+1143¿ÜôBL¬µÀCJ¤ÁëÈ;À5pP‡×ÐÀ:{ô°@¥@ÖÁmH-@–™â"µ.?yW§lý¤?µ^¢¢¬½¹@9–x?'æ@&sg»Ðü¿Ë˸e6»~¿àf·#îÒ¿ä¿ëþ@bF¿äGÊß·¶¿é®‰`‹é¿ì¢úkkˆåAGNFSRQ3FGL J2232.5+1143CTA 102?ïÖa¹¶ù?z»y">á'?tÏ#UrM?z»y">á'?ÎT´5.é€?ÓPP'¾=›?èjÒò´E ?ÓPP'¾=›?쮼ßw|í?¬&èÁ,Ø?ºŠDš?¬&èÁ,Ø?åK""·:?×yíh	?Õh׺'‹Ù?×yíh	?ïÀc.Åݒ?~͸ ìo?Îhƒ¤G?~͸ ìo?§ÎÀr}7?ÂZìd§Î?îƒø§¾m?ÂZìd§Î?ïè{:D0?œ€$²"%?bð'ØB?œ€$²"%?–t—Ô¥?¨\[É×ä?ïL[Aˆû+?¨\[É×äMIXED4FGL J2232.6-2023?î;50l ÀLÓ²VÿÁÀ:ä#åGîÀ<›OÚ2æÝ@ 2ÀD©'V@ÒÁ&¦]?ºz#À8•¿³"F|s)?ù/JUŽ§Î@P@à'¿ÂËr"¬Í~¿è¨nÿ<5»¿ç¤Z¬1¿ÇͼŸ9¿ÜÔWZ¯Îå¿ÛLyÊÇ9AGNbll3FGL J2232.9-2021NVSS J223248-202226?ïþR£ª®?"Ò¡#b?/zÔg°?"Ò¡#b?ïë"©´U?v#N®ú¬ì?dÝVof×Þ?v#N®ú¬ì?ïõÔR¨.?UË¢yÀÌì?TW[–´£ê?UË¢yÀÌì?ïûŸÉ?*"Í'"ºÛ?A€Û~ýµ?*"Í'"ºÛ?ïüªU2?5Áðèúƒ?:¯Õ/ó¾Î?5Áðèúƒ?ï'r‰WO?'UDÈ4vO?‹c|+hœH?'UDÈ4vO?ïðyõó?oåFbGm?_ý'
?oåFbGm?ïàÔ+:ì:?c·Îòñ–‡?o+ÔÝÐõ¸?c·Îòñ–‡AGN4FGL J2232.8+1334¿ì:ðcLMÀB›3ÁÎl	À;{]š
_À<»£IEÄ/@!§â^¯bÚ?ú¯4^¬^?иn¼ W8?¾õCŽu#C?îõ'àh@žwNëö^¿ïþ!¾–©$¿ïEHßlâ?ïÿùëñ¿ÍAÒ2g[Y¿àÔ£éտ̇é­WAGNbllRX J2233.0+1335?ïå
vs?ªLó‰á&?jàõ´†´¬?ªLó‰á&?ïéÒ4Џ?lyfuaJX?f-ÿª31"?lyfuaJX?ïðÙ(zÈ?rAõ£¸'?_øM¡Kÿ-?rAõ£¸'?ïùM­C*Þ?;A·à»âH?JÉK°r9T?;A·à»âH?ïÿ#
SÙ?Š·ÞuŸ±?;šÇ"®?Š·ÞuŸ±?ï˜ÄP7·
?'‹ëTNJ?‰ÎëÙ?'‹ëTNJ?ïê§ø\	?vExïY?eX,ÜÆW?vExïY?ïðië3ȸ?WÓ øœØ?_,)±+¿ø?WÓ øœØAGN4FGL J2233.9-1229?
!ÂÀKV®Bž
BÀ;"k"ÌÐÿÀ<™êBÿY@=^ú·@É?þyòoÀ?Õ<ÿD™7?ÌÈm×ôÉ?ôré+¨$?ý°|Ҏ'º¿ïᕱ­Œ–?ïöUç¡9¿Û(øýWY-¿Ü!YÁèBI¿ì‡Ø¦õ¢¯¿ïÒ@tdUëAGNbcu3FGL J2233.5-1235PKS 2231-127?ïÒyÈÕ¶?tOšç1Z÷?v÷+Pí?tOšç1Z÷?ï¸]ë~ÏÐ?÷ ð?è…å'?÷ ð?ïåÖf²?'\iO?ŸƒE,J"à?'\iO?ïxDMŽ`?uq‰Oâzæ?÷vT×.?uq‰Oâzæ?ï‹6‰ÒÒ?†ÐPÊ|k?2OkI»e?†ÐPÊ|k?îøPA>—H?¦þ‰ñC? zûðby?¦þ‰ñC?î$eœUÐ[?œ-àøx®?­¹¦>–M?œ-àøx®?í¡N011?¤¾ºG>L?²õÆìiô?¤¾ºG>LAGN4FGL J2234.1-2656?ïšK:õ†ÀMî£À9F®×ï?¾À;ãð/¨d8@>|ÔçÎ[?ÿF7õÿÌ?¬¹¤?ԛ?²Râ¥üÿE@4†º™Äb@[ùëñ¿Ö9Tç¸á¿Í6ºý–š¿áÃ^6=¿à÷ÍAìa¿à¿ÓÀí¿åÚI{«AGNbll3FGL J2234.1-2655PMN J2234-2656?ïþ~Œ¼«0?(æ–|èÿ?(1(¥¾Q?(æ–|èÿ?ïîꖷ<?dù%×¾5
?aiŒ@Æ?dù%×¾5
?ïáÏ´pï?sc¤LH€"?n0L*¨X¥?sc¤LH€"?ïÿ£[0ʛ>õ½e3Ñæ=?)9´ä>õ½e3Ñæ=?ïýÓ؄»ç?1Qódïè?1a;ŸÚ›Ñ?1Qódïè?ï¦àµ?šþ?}Ò58éM?†GÒÁGL_?}Ò58éM?ïʉ¨­*=?€‰ŸÎ¬hÜ?z»+ˆn¡è?€‰ŸÎ¬hÜ?ïÿde@‡Á?Ãjç?ú\?sXÆù˜-?Ãjç?ú\AGN4FGL J2235.1-0623¿íô;‹=Ø ÀIʱþë-
À:ßó£Ñ+À<"ÇÝyÃ:@ãܚJC›?ðà"¾ŽE©?Ûy—¹>Ð?ïm8bGõ@æl£—I]@ä(Þñ¿à¥TþŠ	.¿Óiû±¼¦¿ÚÿÔač¿Ú®b¾ç	¿ð?ïÿÿÊPËAGNbcuPMN J2235-0623?ïÖûQš|n?•›2OL"?t'W$SmM?•›2OL"?ïêO[–?pòÚxh
ß?e°ñ×¢#?pòÚxh
ß?쮶-ÆY8?¥œCL³ ?ºŠN'Í6C?¥œCL³ ?ïð™G[«š?QžIQB?^Íqld¼G?QžIQB?ïÆ,Ä-õ?X"®·Ò®?|éÿ;u©%?X"®·Ò®?ï¡ÓD59?',<|§á?‡‹.ö!TÅ?',<|§á?í«1r¥?¡šçª9­?²£‡¦â^X?¡šçª9­?ïç-óД$?fü7¾?hÒ4ë;ò?fü7¾AGN4FGL J2235.3+1818?µu¸.À@ìƼèS;À:i"6ÆÀ<h·'"…@ğ+ÔÅ?ÿƒ†Üþ?Ï¡Ñv¹?ЙäB4Wö@RóݲÎ@:äßJ¿Þ®ïÔ;V?ўY<1^¿ãÜÝ¡0fпÔ<_p#¿ìaÈ"n·¿ïÁmž%øAGNbll2MASS J22352860+1816356?ïôî}æN˜?TtêÛÿc?V#¤ÿµ?TtêÛÿc?ïàˊ¡?pc)‡?o4v"Úë?pc)‡?ï! iµ"?ƒR Ñ'@¦?‹÷·ïárù?ƒR Ñ'@¦?&‡TXÙ?a8b$ÀÝ3?€Þ^ã'Õ?a8b$ÀÝ3?ïâœi'E?n%o½0"N?mc–¡c?n%o½0"N?ït6¥¥ãÌ?™ƒ¸Ë|Ú`?'y+N³"t?™ƒ¸Ë|Ú`?îßÊX? î"hýÉ?¯'\²±¹? î"hýÉ?îíæ½¹´l?æ©!3òÅ?¡!""¬ë@?æ©!3òÅAGN4FGL J2235.3-4836?Ün;-8ÙÀL
×6&-À97½8SLÀ<YÑ쒛@¬Ê"ùT?@o`àëh?¤Ý,ÁT¹?–ä&¹/ê‡?æãôÑΔM@Ÿá∠οÝR°[Ò䔿âÇZ!‰'¿èý'¬¿å"]àZô¿æ4²G^¿áHrÏCAGNfsrq3FGL J2235.3-4835PKS 2232-488?ïû2%3?y{¥—ó‰÷?C5Š"XŸú?y{¥—ó‰÷?ïöÕ/
É?W*/ÏE?RäV \º?W*/ÏE?ïæì?¦*™?qÎ/"o>f?iÀctNõ?qÎ/"o>f?ïÿµÐ1\>ùL/çýžô?‹ý'ç–>ùL/çýžô?ïÿ³8žyu?
 ' G¯Æ?1Ü9ë:Ò?
 ' G¯Æ?ï߃ÃÄeu?s¡=¬MÆE?p>?s¡=¬MÆE?ïÝêýöv¦?{sʆ°5£?q

óù2?{sʆ°5£?ïÿnÔ/Rå?ä*ûø¯j?%y#¾ßA?ä*ûø¯jAGN4FGL J2235.8-3627?ïñ"G€zÂÀMórq6¤À9}'OH<°À<\²ò03¤@§Íęw‹@Qæ­j1?®Ø\fÍ?³©/¶@ð{xFb»@
C+ò!?ÝC›=]¯¿áÜ®ÙÄ­¿ãOx¶Ë¿ã	U~·–¿æ`ai§d¿ïýüðüAGNbll3FGL J2236.0-3629NVSS J223554-362901?ïúKðSJ?I*;<ÛX¿?FÐ@ˆ¹¤?I*;<ÛX¿?ïì洁–?jsS)ŠÍU?cì~X¡ˆ?jsS)ŠÍU?ïË°¯#³R?€òe¦`œ	?z'¨}DžÊ?€òe¦`œ	?ïëõéÈþY?Q8´ÕÚj?d
DÀj?Q8´ÕÚj?ï÷…^½êK?UQta¼?PõBÆ#êY?UQta¼?ïrXÅòp©?—H'	`;?'´ç<Š€ê?—H'	`;?ïµL¢í©?" ǀ±P?'¬×t%­Ã?" ǀ±P?ïÆß¼­^·?k&|Œ‡©'?|!ªe?k&|Œ‡©'AGN4FGL J2236.2-1706?íûµ³çµÀLŸºˆ&ªÀ:'Û ¥&–À<k—€º¥ƒ@øےbm³@›ß>¿Xp?¸2Ó	'¦?¹•b?äض%ö@<ŽP».?ìÎø@n?¿Õe;Ãûm¿ãÝK8)'¿äúm^Ó!¿Û9æ@;Yr¿ç—ͤ?»AGNbll3FGL J2236.0-1706PKS 2233-173?ïö»1³›?Ff¢ƒë°?R‰œ}Lýw?Ff¢ƒë°?ïí?¾±Öý?eó×מ?bÀA<K
ñ?eó×מ?ïٟVz"£?qô×ø`ä›?s0T½æº¾?qô×ø`ä›?ïèxC!Ÿ?RW‡ý˜"G?g‡¼ô{á"?RW‡ý˜"G?ïÊÙÏá÷y?q)ŽoË9?z"£+"?q)ŽoË9?ƒ8Ñz?Š×î¹½˜«?‡ßBù­^?Š×î¹½˜«?ï¡ÊRì{?‰¹DBö?‡zde©T?‰¹DBö?ï¬Â¹¬I?s!Á6d­?"ÏQŠ¬ÙÍ?s!Á6d­AGN4FGL J2236.3+2828¿á¥eeñ‡¨À9¦M;òõVÀ7Éá|‡:À;8œÿ¨@k'HíYµ@*ˆïþ*=?˜N𪢀?ºÄñŒܺ@ Ú£ßm¹A@@Gbj-p¿À¨c¶Þ£å¿àz¡†Íå¿ãwœ¹ßŠ?¿æ#… êÚ¿èqJÝõ¿äy®ý®ìèAGNfsrq3FGL J2236.3+2829B2 2234+28A?ïôžÝóˆ?qÙ~ïé?WüÂ.oë?qÙ~ïé?︞{šnð?–ˆ£=Œqv?Øaô§ë?–ˆ£=Œqv?ïˏô1ô"?'†g"Ý?z8ÿÃ?'†g"Ý?ïì@tܘ>?Vóu˜†‰?c¿‹3åá¢?Vóu˜†‰?ïî¡%üû?`]h5%€?a^æ¯gÝB?`]h5%€?î·üçFÌ?´4uª0}'?¤Ž°2gzE?´4uª0}'?ïÉtzr¯A?ƒTrðå?{EÂÀyR?ƒTrðå?ï'jCsOá?€'š¯â
?eo#,£?€'š¯â
AGN4FGL J2236.4-2309?ɟìAå±(ÀM¥ÈÉ2
™À9á^"ð•)À<drr
c–@l#¸ìÆ@P%çñ?»D?JÑ-?¸ŸŸ˜O?õ2cʪ³@uåµQ¿ãSe¢òð¿âµl]÷,¿êž€‰'\¿èl7`¿]¿ïÿpŽ• ¿ë@ðàþ2 AGNbcu3FGL J2235.6-2319PMN J2236-2309?ïü³ö£F'?1[:$`ÅG?:`Kí°ÇZ?1[:$`ÅG?ïìÞØ	ŽA?q|y[_D?c!(‡5?q|y[_D?ïʹ¡™9Å?{OáGÏF?z£/C1QŠ?{OáGÏF?ïø"üS£?>®"t_?MìZ—%?>®"t_?ïøõüŠÄX?GÜ'½¯A?L(
M±2?GÜ'½¯A?ïªóP;¤?ˆå¬ÉÆ?…C+þÕkS?ˆå¬ÉÆ?ï¾/Å.a¬?'ª³HŽµ?€tÃÝÒé?'ª³HŽµ?ïß|%P­©?d&ÀÔ´?pAí5MÚ?d&ÀÔ´AGN4FGL J2236.5-1433¿çA¢h0|0ÀL›ºÜ	À7™šFgÃ^À;R; g@Úô	Q¸Y@"3ÿ
z?–A…s"?²-í_O¬ø@Ï⾦™\@çv¹iÄ¿ºþÜ>"Ë¿Ý 뽨¿âÔ"Œò¿⹁@‡Y¦¿æ€ƒ}Îaø¿èי¿"9áAGNBLL3FGL J2236.5-1432PKS 2233-148?ïùÑ3"k?KÜnD?H»4_]Q£?KÜnD?ïã¡뎄?zŒB+?l^æU
#¿?zŒB+?ïÛßG<™?y»pÂ'‡Ï?r~Hs÷s?y»pÂ'‡Ï?ïÿtê/*²?+3¶z?b½1nƒO?+3¶z?ïûœBK-?@@AÈís•?AŽ÷{`lQ?@@AÈís•?ï…Ü›Õf­?›'éÛ¤¡£?ŽˆÙ…Œ½?›'éÛ¤¡£?ïâœëËP?zoU£¢"]?mcÅZwÑ?zoU£¢"]?ïþàڏœÚ??è/T
\?!òZ6É??è/T
\AGN4FGL J2236.6+3706?ä,8 /ŠÝÀ2c¥]:ÉÀ;A¹'ÔZ`À<šE'±H@!þ75Ì?´?ü<b¼ºh?ËóÍ–&?˜ÃOܝ`Š?ÏÃYª¹Ò@k,†›»?å!͗¿áìv0í¿âeˆðÔê¿ã<`®kŽ¿Ëßõ½‡¿Â"3£ñaWAGNbllNVSS J223626+370713?ïÿ˜•K_>þ•³n?	úK–Êýþ>þ•³n?ïò‰ÕQN?aågHD¯‹?ZìU1—s?aågHD¯‹?ïø°oŽ?[[dƒxø?M?Ím¶å€?[[dƒxø?ïþlk|ê{?¤´&$¤m?)9Iœ/ã?¤´&$¤m?ïÿ±$"x·?[¦™ù\?¶Üßfã?[¦™ù\?ᅩˆl©)?‰2gË9?€Ý×Ç1Ä?‰2gË9?ïúÏ¥«[õ?YÀüçÌn?DÁjBÎt:?YÀüçÌn?ïúŒJs
5?=k¸+FR?EÎÕÑc(Y?=k¸+FRAGN4FGL J2237.0-3921?êF낫§ŸÀMË~dž<À:–VîúÀ<ˆL×I''@léú=|@–Íl.ýD?·üß¶´]?µy™ßd©ù?ûÖÃƓÎ@՜9\-¿â¨+BNC¿â«ï§Ã(¿æ~¸—·¿ãÿL±‰zh¿ð?ïÿÿ>¹úAGNfsrq3FGL J2237.1-3921NVSS J223708-392137?ïûÞjâ€?UÆHÛT?Cˆ…ÛƒÂ??UÆHÛT?ïëzd °?q‹à.b™?d…›ÆH%?q‹à.b™?ïZrÊ`œ?'F]_ì?"±¦Ã³$ƒ?'F]_ì?ïÿ¸ˆ£>ö1Ò MáY?ߣ2‡ïK>ö1Ò MáY?ïüÊúBYt?GšGV:?9¨.Lܯ>?GšGV:?ïtŸ†óö?™²5Åû?'l4à¹<?™²5Åû?ï‹#ÍÃ?ŽÜgDh×Þ?7ˆXçh?ŽÜgDh×Þ?ïÿKRlg?>‹ùòÙ¥?•«áMþ¼?>‹ùòÙ¥AGN4FGL J2239.2-5657?ÛÙÁ†?ÀJã—­À;o†§NŽÀ<ê>Ä`î@cŠ!+ž¿?þ^ã MèÁ?Ù%™A¯ø¬?ÐG¤"Y@Ž?ù–p4Eê?þï~'£2?ï²µ>»§‹?Š8=3<B¿â :<½¿á°ìœuìì¿ïêë I÷p¿îå[n»Ÿ~AGNfsrqPKS 2236-572?ïí¿Òy›3?Xjtdï)?b@-A¬­?Xjtdï)?ïÙ£ÿŸ?~‡y+É:?sx­ÿØg?~‡y+É:?ï2ú³\ZÁ?‹†"mà¢$?™ ©—äCÔ?‹†"mà¢$?ïÀ%šz·?bÀgâ…ýK?í{ ä¬\?bÀgâ…ýK?ïÖEG'¡?pIò3,ü?tÝ\W:ï«?pIò3,ü?ï"õ׫š?¡³L%Ðþ?ŽÂ¼WӉQ?¡³L%Ðþ?î16¾Fç?šÏ:,¥=?¬ï•Ó_?šÏ:,¥=?ï)8…Ç?‡È¾¬?çá?Ÿ:ݓÇÝ?‡È¾¬?çáAGN4FGL J2239.4+5130¿énì`ª©À¾ºñ6;À:!K,F°À<N0å{@´Î3@*y]¹ïz?Ç!'al¯?Ó]‰Þe¦x@+‰>@+±ÐÈ?å+$;H«j¿Òë!Cœ¿ænÚs~|Þ¿éÑÇ"hà"¿ïÿÅ}M2¹?áEUt¦›AGNbcuLQAC 340+051?ï´älëT'?°ÊÃI´>?'ÆäÉúO´?°ÊÃI´>?ïËUd-?~r'Ž]Q?zUMìeŸ?~r'Ž]Q?îÞ-lõ¡­?'wc•¤ã?¢)0¥å,?'wc•¤ã?ï.'ÿ­?ràUq÷Á?;ˆ<g?ràUq÷Á?ï
©k­?#æŸt?ž^ªÙ}¢R?#æŸt?îž™øRü?µðâ˜Ëo?¯Æ`zÐ<?µðâ˜Ëo?ꓒLpÇ?®_8ˆ}T¤?űµúÎ<ä?®_8ˆ}T¤?ìf[=µº"?£â6	Š?¼Í&R+á?£â6	ŠAGN4FGL J2240.3-1246?֑)"D ÀL
{é…jÀ;WÓpóˆÀ<Œå—ží–@ åp…ùÿ‹@?ßÁœ"?ÃCeÛQ¿¹µ	a¨'"?ò…Šƒ| ã@ÈæšSRã¿îéºy
2?ïœ&Üã›E¿ãŽñŸêì¿ã¶,ýx¿ßS€Èп¾`ÍöŸAGNbcu1RXS J224014.7-124736?ïüHÆ9Ø?4Æ=ØEF??½»Ýõ<Ð?4Æ=ØEF?ïè~5(ð~?js‡Å?gËˆ¡»?js‡Å?ïâ`±µ^
?n¡CùùZ?mŸNaÿMÏ?n¡CùùZ?ïók*#Ã?G¼Fø(ÏA?Y)«wÍùì?G¼Fø(ÏA?ïï"òC\?Z´âN*Ã?`l
Œˆù‰?Z´âN*Ã?ï`ɱ0Ü? 'c=
?"ðÍI€o? 'c=
?ïÛ¿"mk?u¥Â(ýLä?r =¨N2©?u¥Â(ýLä?ïˆ1:ƶ™?"…š+?ó±@"é¸?"…š+AGN4FGL J2240.7-4746?ë鍁w'ÄÀL¡R}ÔAÀ;Îj[¾mÀ<Íëýê|
@ð¼~ ïÏ?ÿÌQ—¢H•?ĸ[%À"?"bk¸"b{?Ð2ý›¡²@ÿtHQRƒ?ïjà"'¿ë£BÄ ®¿§ãØ_°J¿ãiÀùYó'¿ÙpÁž›a¿âÇP÷iX‰AGNbcuSUMSS J224042-474733?ïüôôÍá?B5He—	×?8XZñå?B5He—	×?ïö@0:'?W…•Tµ>ß?S J>Ü?W…•Tµ>ß?ïìBMØP?qDݘÍ?c½²	sbv?qDݘÍ?ïýÆÿ¥´|?c¦¶A:?1Èê\äN?c¦¶A:?ïý›÷a9?2ØçÑ´D}?3 HÛ6›"?2ØçÑ´D}?ïۇ8ª&Á?tÔ#c¾^?r<c¾*oƒ?tÔ#c¾^?ïó)~HÍ?kP'é#&?Y­´5–V?kP'é#&?ïúÔø™?:…@ cáŒ?G˜°²…8è?:…@ cáŒAGN4FGL J2241.1-4122¿Í
a"ÀÛcÀMä|"µÜÆÀ;úd­(—À=‹Ydö$@"'ÌGÂ?àZ«n®4?ë
¡äÁ¶?ïÿ ^¯¸À?þ¥nij&å?ûmQÇÈÖô?ï¢b€}¾È¿éªÀ2‹¿áÓ¦¥ñ–±¿ÊLœ»·ü†?Á.èävã¿æ)ù˜Ý±÷AGNbcuWISEA J224103.56-412155.5?ïÞË:õt?|ÍßÏ7{?pšuŨø?|ÍßÏ7{?ïï–t\Yƒ?l™¢mp£Y?`i‹dm¬ó?l™¢mp£Y?î¹+)úOg?™´¸f¢Y?¤mM_"'?™´¸f¢Y?ïù¦|"‡·?@zt݈Y`?Ift÷Vç?@zt݈Y`?ïõ4šõå?`ZŽ'´»?U–ÌH
5Y?`ZŽ'´»?ïÆ_«ó?†.†tO'w?|óPGR¾V?†.†tO'w?ïN¤ûnî?'õV°p2³?–+`‰‹74?'õV°p2³?ïò¯k×®A?b¬uy‰ÅÅ?Z¡(V"Ýä?b¬uy‰ÅÅAGN4FGL J2241.2+4120¿æ`œ ½­ÔÀ.bdä†&öÀ9×Ϗõ«éÀ;ç¼SØÅ)@Bðòç>@n?©c;?¶‹&å#ø¿gï¾d5Pó?²—Ð¸"±@wwZÕ?ëߟ¢È…¿ÌÖÒI¹\ƒ¿å	€¢&Ûâ¿àvé€â"‰¿âS¡2OB¿å2_ê pAGNbll3FGL J2240.9+4121B3 2238+410?ïýâGO9?"Ô½à(Õ?0ë}
ççë?"Ô½à(Õ?ïóÔ1+WX?]üˆ¥ü‰?XWžÅo¡?]üˆ¥ü‰?ïóª¢&?_Éìä[?X«ÌÄÃ÷?_Éìä[?ïö-J2v?;öÿ0@$;?SË¥v™ÔÆ?;öÿ0@$;?ïùø`ñ©È?A£—Õ$?H{:B¬º?A£—Õ$?ïÁBÔL.=?‰.üI¥H?^•Åû%"?‰.üI¥H?ï솠‰÷?pT-E´È?cy_ßY|?pT-E´È?ïâ§Q_?Yӛ,õŒ?mX®€Ós?Yӛ,õŒAGN4FGL J2241.3+2943¿ç
-žµÀ91jœV|À:ÂðBóš—À<{""i·T@ q/ÓØ.Ö@óøUӍ?·IËù")¿·ó¡!ù$@Ú~<F@üU8k¬K?Õìmçd'È¿ŠðÔqlù¿å×4ó&Ô¿æä>ÙY£
¿Ò×'™¡ý?¿—Éà´5QAGNbcu1RXS J224123.5+294244?ïÿÃð@?¹tŠÉ?gˆ=9f?¹tŠÉ?ïíɲ2þ?i!Ç2&–^?b6M¸ÓBH?i!Ç2&–^?ïñûÿD2?e2wƒû`?\	ÎF/Ë[?e2wƒû`?ïúj™žCš?1S9d#.?FUš)'Ê?1S9d#.?ïþùKl ?,Ða¾ID?. j™QüF?,Ða¾ID?兀'Á?~;8H‡?…øÜüîô,?~;8H‡?ïéê"UYp?sLc
G˜?fk§æßÙ?sLc
G˜?ïÎÜuGô?oAˆ-?x'Å{ÓíŸ?oAˆ-AGN4FGL J2243.4-2544¿ïÜJ"…]oÀN²]yЦÀ8ó犾4"À;·ÇHÿMS@TXD9ÀÁ?ÿú¨W¢~E?ªñ#
Ì?ÀÝU@w­_I;³@S¥m¼F?ïÿÀà/€ ¿Ù?e*)¿àaâއ	t¿ã+Ñà2_¿çÌéhM¿Ù€/»."¾AGNbll3FGL J2243.4-2541PKS 2240-260?ïó«áù7m?eñï.Á|?X¨;ÙW<?eñï.Á|?ï¥b›ç¸È?"Õ{®2i?†§Y	j?"Õ{®2i?ïpà[†Ï?—?'ãô"c"?—?ïD¯,±l}?y‹ñEa8?—jiÒpj?y‹ñEa8?ïx]¬%?—eþ¢ââq?ˆ¡èŠ§ë?—eþ¢ââq?ì{fÛ"ÈN?ÄbiTŠúM?¼$É&齍?ÄbiTŠúM?îÛð1¼÷©?žC?½&³ë?¢@üßåy?žC?½&³ë?ëºÊ¯ê?§Í×w–Q ?Á×Ñ@W'?§Í×w–Q AGN4FGL J2243.5-3931?£Aœù«;ÀN`:!cýÖÀ:‹ÆÞÀ< 7Ǫf@½ëf?úí@w❪?ÃQsûz_B?¼BÎÜãÆ?ö¯Äcq¿`@E3²_
W?Ŕ€ãÀ.¿äbžÍ¶¿å$¨ Eæ¿æy¦µ¿è%Áۂ¿ïýݱ žÜAGNbcu3FGL J2243.2-3933NVSS J224326-393353?ïÿ''Á2?‡µ·™Äa?MÔ%û$?‡µ·™Äa?ïôƒ¯h?[µ¡@ç?Vø¢B$‡³?[µ¡@ç?ïã+o*Á[?v´eüÌØU?lԐ¹ÁÅA?v´eüÌØU?ïú\Ö^‹?1Õ$ö?G'Œ¶w8#?1Õ$ö?ïÿ'•Õ?âò#ù?_²)»-3?âò#ù?ïÔÄAQȹ?v߆™$êF?ußGý[g?v߆™$êF?ïæÔ0!
Ÿ?rïQrÀ'.?i+ÏØ(±?rïQrÀ'.?ïäÒióÜ?^ ݅€¬¿?k-ù҅C¯?^ ݅€¬¿AGN4FGL J2243.7-1231¿æX«ÎâÀL_9&A³À:pûëžÀ<7ªËñ@žhJí6@‹SB3'?³ª$>®ç¿±±ß‹–K±?ý÷½#â]@~矕¿âu	—Xw¿éxHÞ½¿âD­Cš‰"¿ãS{ýýFg¿Ñ)O¤Øçã¿à³ã'/ßAGNbll3FGL J2243.6-1230RBS 1888?ïúuñÚß?@R—Õ†É?Gê'iß6'?@R—Õ†É?ïèÁŽÄî ?t®ôgK	?g>q?1h?t®ôgK	?ï莡5«?nX¶L6¢?gqûƔc?nX¶L6¢?ïòÊk1ì?Axú|rÎ?Zké"Q׎?Axú|rÎ?ïÜ,;ÐÄ1?n¾,jÏ?qéáö¡§Æ?n¾,jÏ?籈+?f%7—Òâ?Œ[.Y+?f%7—Òâ?ïÎE7?€òBIF ?xÝdš4ô?€òBIF ?¡l)}?~ÚN<×'?\פõ ß?~ÚN<×'AGN4FGL J2243.8-2510¿Ñ訁ÔÀN¯'Àa"À:~-o}À<
qäHêU@M¾—@iÒaaCè?ؤó…?ïÿÕm…>™?üªáÀyØ@`œ¤ç¿Ôúҙ•gÜ¿â ç×Nl¿è±¸¿y¨
¿í•
È?Ÿ¿»{šâD¿ïûX0B½ëAGNbcuPMN J2243-2505?ïÁê'ýÀ'?•Ë߆Û?
¶máï?•Ë߆Û?ïíëš~'?we5–gC‡?bçz%Á?we5–gC‡?íWð"×	V?¤ò™â€?µ@~èÙÁÕ?¤ò™â€?ïù5"Š¶Ó?@¶X˜WŒý?K)°ý£œ¨?@¶X˜WŒý?ïÞFÿ:î?zçÉ ô'û?p܀C'5+?zçÉ ô'û?ï¤ú¹w¸ý?	ðf&qü?†ÁQ›2ˆÚ?	ðf&qü?íg;üÉ?£'¬š¼Õ?´Æ !$ì2?£'¬š¼Õ?ïå¤zi?g¹ùÃº?j[ëJ}²÷?g¹ùÃºAGN4FGL J2243.9+2021?ÇêK£"ëÀ@®÷S½À7ìõì€Ç;À;5ìlø@L·
Gç?ûrÀç¼<\?þÞmÅ<?µ®_4ª@qØ¥H#…@.G«æ"^?ËѺÀ/Û¿¹^f'±¿ÙrԞReþ¿ÛØz™9¿Ý¥SŒ¿âpY.oAGNbll3FGL J2243.9+2021RGB J2243+203?ïûøQ"y"??ׂÉ/?@¸¸"§]??ׂÉ/?ïÆó®Ÿ ?•}`XÈS?|÷‡Ï?•}`XÈS?ï"< ÍÈÿ?ŽÏ*¥9Ë?Šð×Ý»Ì8?ŽÏ*¥9Ë?ïâQöº(}?Wª#n]ðe?m®	""n?Wª#n]ðe?ïõæ-"X"?S¼è'Œ?T3¤U]ø'?S¼è'Œ?ï´Z\D?²ïWë?Ÿét²¶Is?²ïWë?ï¨ÈœÍ'Õ?¥ß*Ðì ?…ÍØÓz½?¥ß*Ðì ?ï‰õӒtó?zTø*¢¯?'‹ƒ‹3?zTø*¢¯AGN4FGL J2244.2+4057¿Ü1XÀ/šw@Ý@À7zw⏬±À;3R­Kþ@¿AùŸ"@4ìÁ^ځ?"œ˜ëZ?¸³7¥]È@$©?)
»@ »Çö|?¨+Ø ¿Ýh܂¢\6¿áóìáÀ#ò¿á0%⒱ɿæÉñ…é¹m¿èÏ|_LØAGNfsrq3FGL J2244.1+4057TXS 2241+406?ïôHè.ۓ?WôXï:Ï?Wn/R'éë?WôXï:Ï?ï½ñªI6¢?"KÜ°I?€ƒ•pu?"KÜ°I?îזŸ
¿?ždŽá4?¢†–‹"?ždŽá4?ïý‹–'6?7·³CÓ¤?3£N=}.$?7·³CÓ¤?ïé¤[5þ?`ÅÝ@I´?f[¤Ý?Ä»?`ÅÝ@I´?îÿ¿á+ÿb?±TË=¾m? îðÚ?±TË=¾m?+,Ì?'ªO¹¢é?Wúµ4Í	?'ªO¹¢é?ïõ¾?;"?PWöú|i?TƒpØ+7?PWöú|iAGN4FGL J2244.6+2502¿Ì€ZÅë©~À=‹T~–À:ÆcQÞïåÀ<"PP@líañ3?üðiϘY?ÑÖï»dD£?ÒòõÀáÜÿ?ÿõ²ÉìH?ùÿ¥è¿å÷É?¤…±¿ÑÑðã'pÞ¿ÞçIeN¹L¿Ø£¹bâ£N¿äáâ¾P³!¿ïÿýF\IAGNbll3FGL J2244.6+2503NVSS J224436+250345?ïð¼ÓQî'?jë	»X?^†YÕ<?jë	»X?¯ãÕI?'ôçü†¬`?ˆ•SùL=¸?'ôçü†¬`?ï‡[öÃ8?Š&LáSC?zHa?Š&LáSC?ïQƒ!÷»?v(Ý»zɄ?•ÌO"*¢?v(Ý»zɄ?ïè¹9>‡r?d}ø'uú"?gFÆ÷v?d}ø'uú"?íÜÈc®L?·ê/nüŽ¼?±¼à ³!?·ê/nüŽ¼?ïGԑ«þ:?'tî2…àÀ?—mÍïÔ½?'tî2…àÀ?ìX¸ÓƑ?¢<!‰°k?»•:9aËw?¢<!‰°kAGN4FGL J2244.9-0007?ïN=_ÜßjÀH­Üa•FNÀ:ìj`Æê5À<CãÎq»@VU7«@pÜ¢b–?Éç¨ìMñ?€}:	Þr‰?³¤ÁÀÕ?ÿÞ½:2¬?ï*2‰}ÿæ֙ŸxÖ«¿â^éÐÒk¿äjÜs­¿åcŽz¦^¿ïù?A3|AGNbllNVSS J224448-000616?ïú~¬-p?FÏàb; ?GšG:ۊ?FÏàb; ?ïçÓòÂ?jb{EÖ¯?h,
´™¯?jb{EÖ¯?ïãè?D
¡?g!ŒPˆ"?lÀ‰'I?g!ŒPˆ"?ïãHŸßŒv?POš"6†?l·`öª"?POš"6†?ïç "ÓGC?eÃzNà?h_Üð?l?eÃzNà?ï†Ü	¼~?"+]î÷Ñ?ŽHø}àŸ?"+]î÷Ñ?ïÁÕ¤L?'*#›?|Í[Â?'*#›?ïmWZ@#˜?}öÊÉ-?'U·û?}öÊÉ-AGN4FGL J2245.5-1734?ëˆå3ö҅ÀMºõýG¾ÛÀ;Œ8ap]`À<Ô/[7^;@!´oˆÎñ?óÊíêSÆQ?ߙ«¢°™?ä‰ößÅÎ@¦-['Ý•@¸"Æ©r¿ïÿSg†!?ïô…¾Eu€¿çÃÉîËû?ÈíPÐÒëË¿ÏÄãIeú†¿ïöºÂM¬AGNbcuNVSS J224531-173357?ïì{Àã?iN	µ'—?c">ãE'<?iN	µ'—?ïÒhN#ú?Œàh´?$h?vËðLjä?Œàh´?$h?ï;·Rßm[?‰:ò\bÞ?˜‰›{N³?‰:ò\bÞ?ïèHg¼–Ž?YŒ{²«žâ?g·˜sƒú.?YŒ{²«žâ?ïà›Ä…ð?o¡ú̜s¼?oød(<?ç?o¡ú̜s¼?ï݈SB•?®ÈФd?œDNî¸uv?®ÈФd?ï)"—ÉN­?•°"xç?šÛ­\h?•°"xç?ï®`cÿ.?€4êeây‡?"gæù³²?€4êeây‡AGN4FGL J2245.9+1544¿áFùF°òÀBµ‡aˆ±À9ȺÅ­À<£Ä•Æ¦@ 8`Á¥?þ^ŠÏÒ;?ºÎ¬ l?³[;ùç?ôõ]ʶr@
ÌÕHq]æ?îZÌiÐ~2¿çsø :G¥¿Øýç!¿Ü/›¤
᰿ᆚï/:¿Þ!ƒkáAGNbll1FGL J2246.3+154987GB 224338.7+152914?ïþÜs!Ïw?Å;ŸB™æ?"8Ì&Ô¥¥?Å;ŸB™æ?ïíœLôœÂ?e4çy‡'•?bc²ù…F4?e4çy‡'•?ïù3gáe¶?>"G	30Ñ?K2`µÈÍË?>"G	30Ñ?ïö`=ú¯?<ÎG¿Ïx\?Sñ?²ÅR?<ÎG¿Ïx\?ïþ(ÖI3Œ?#¿íÒâKî?-r™
Eº?#¿íÒâKî?ï©â'¸?ŠÅ7–j?…¿Çx'ù?ŠÅ7–j?ïøùC´q?aȇÉ݌?OÐ^B	?aȇÉ݌?ïëT4™?R™Þáï?d«þë"ÎX?R™ÞáïAGN4FGL J2246.7-5207¿ÔPW=K†ÀKê¶â—À:ï/éÁÐÀ<E³Æl@!­#>ô\‰?úƍ«?Å<)¦íj&?³]&¡ª_:?ïÊi²KA@˜»ûÄ1¿ïÿÒ†ëA?ïmMá4c?é°Sº'7¦¿ÀãÛ\1¯%¿âñÝ}t¿¡^ÿÝp^AGNbcu3FGL J2246.7-5205RBS 1895?ïÿ™
">þÄ2iÊ¢
?	¸û-£B>þÄ2iÊ¢
?ï÷_â,Ÿ4?QµÙÚ<" ?Q@;Ø;÷m?QµÙÚ<" ?ïô>Œ"ÝÔ?b¡|Ž/Pû?W'æƒH?b¡|Ž/Pû?ïüÌ4T# ?+Â3Çõô?9ž^MG?+Â3Çõô?ïÿˆ ¸Ì?ê‰àÆ?
Ûì¨I6?ê‰àÆ?ïÚ9—Pi?,öÑØ£8?ròc(©~?,öÑØ£8?ïõ	)Izr?fY'0©™?Uí­Ý¾J ?fY'0©™?ïûŽ®P'F?;fÏI:Øg?AÅFfèñ?;fÏI:ØgAGN4FGL J2247.4-0001?á‹9ÌvÝúÀHÞí¢/jQÀ9ÍÊ¢P!À<õ¦	ê@aóA€¨Ý?ÿÖxG9zu?¼¬†hÍ?±©`­Ç?ô=Òä>š@Wëî%7¿êÿ‹ /}¿µ~#qt6‰¿ä‰!S6ß¿Öký¼ug¿ãË=€"¿åv˜B"ÐAGNbll3FGL J2247.2-0004PKS 2244-002?ïý1C?/1òû/ºê?6w.›Éa?/1òû/ºê?ïí#Yvhè?c6Qš*Nå?bܦ`[ÈC?c6Qš*Nå?ïôÛï!û?]œÜƒÉڜ?VH!GÉ{]?]œÜƒÉڜ?ïí8qOg`?JoKÐê™?bǎ—Ûoý?JoKÐê™?ïúE ÿ6?@ÞmíKØ°?FëÁÕ?@ÞmíKØ°?ïÌÝÏå—?ŒOŹT—?ˆŒÈ~H*G?ŒOŹT—?ï™FŸ?l]ïݐ™â?aMqô±?l]ïݐ™â?ï¶ë>
=?q¬omi?'x3ìL·?q¬omiAGN4FGL J2247.5-3700¿Óà6ÆÀO쿱[WÀ;q?ÊjåÀ<É(˜¥}Ó@+LOŽÞ€@›m´Zæ?Ö>‡$L?¼oU£J?àhÄÓTÑ?ü["ìÝ¿äCt^v­Ü¿ê•êMT¿ã1¾kàú¿á
ÀþŠÓ¿ïÿßHÐSj?ïbŒ•AGNfsrqPKS 2244-37?ïÉ>Ÿ†o?''KBxf?{` M,£?''KBxf?ïÖ,ï2l?¨²?téˆ}f)ú?¨²?î Ô7"É?˜˜zt`04?¥ò¼ƒPu?˜˜zt`04?ïð,Ë›r?Níåu4t?_¦jvºB?Níåu4t?ï𙄏¶?g7ß®f†M?^Ìö‹]¦Ú?g7ß®f†M?ï	´‹Ú¶'?§òl¯ÛÄD?žÉnÃÏ?§òl¯ÛÄD?îÌêP¸¡"?šÛ5ÇíR?£1Z÷傻?šÛ5ÇíR?ïjRC;5ƒ?‰y†!ïH`?'µ·˜™O®?‰y†!ïH`AGN4FGL J2247.8+4413?ïb…-fæÀ*'||R`öÀ9ÄÁA® À<iÍ#3â@!-þËøf"?üb»frû ?³,qMB?Œ#nUY_?ڜb6Uýc@hùÔî¿ìäo¶q@µ?ï<›'Á^¿Þ':_w^Ü¿ßîHÝêVv¿Ízƒ~Ы¿ÙlƒKy{AGNbll3FGL J2247.8+4413RGB J2247+442?ïþkµ°¦?%ZÇb¹Ê?/ùGz£Y?%ZÇb¹Ê?ïôÖÚö9?Xtd*¸ð?VÞRUN2?Xtd*¸ð?ïì5cË<»?p¹lܘåô?cʜeí?p¹lܘåô?ïóRt¹\Ð?D´I{4=?Y[$Ò@Ù?D´I{4=?ïú|#'?AÀ~íœ?Fúàz
?AÀ~íœ?ï°µ´z?'¦àZò_œ?ƒÒ¹l'~?'¦àZò_œ?ïÐqN:º?'¨(šOó?wðGjÀš½?'¨(šOó?ïàB{á³ö?a°ªŸ&ԇ?o½ƒðñ2r?a°ªŸ&ԇAGN4FGL J2248.7-3235?ÔP…²¹	ÀOyI@»±òÀ9í|7‰À<iÆú$ô¬@htbÑ@⩓àß?µŽ]ü4™?£bÓd÷?êBlA@\gç'l¿Ð㔤è,O¿ç$`ãð€¿é†Œa!Øî¿èœl^Íì¿ïÿÿ&¦³?ïï?ôÕ÷AGNfsrq3FGL J2248.6-3235PKS 2245-328?ïüX›w•8?A_Ø'ߢÜ?=;"¥ë©¤?A_Ø'ߢÜ?ïíÎ+¾í?kcہÑgð?b1ԀKÈ?kcہÑgð?ï»;"7Z?€ì9Ќo?:q+Ã}›?€ì9Ќo?ïþ^ˆfÊ?Ö&)r†?*€¶²+?Ö&)r†?ïýR®£–ó?:Å:u"?5jŒìs‡Û?:Å:u"?ï£nÆðÚ?Œg7¼ö?‡${@…Y°?Œg7¼ö?ïƾ,b?'JzSÙs?| ð†«w]?'JzSÙs?ïøm
Uª"?E±…'­}+?NKÖdÉ?E±…'­}+AGN4FGL J2248.9+2106?î£ëâ32ÕÀ@±Å3À:P.ŽˆÄ_À<[6@KAqåK@·ÛnP?³?ÂT¶ø°?´÷îc c?ñhãï(Ah@V0´RØ?ïS³çc¿ßifËæó¿¿ãÊ
æ
³¿à5ŸI[ê¿è¸ê—¸ï¿ïýc¾yåAGNfsrqPKS 2246+208?ïý´Þïd&?#º(¥¦›G?2Y"¯!?#º(¥¦›G?ïîîÅÅòh?d/t—ž?a:MKgÓ?d/t—ž?ïòH6Ðv¥?Yh°–ÖÞ®?[o'·´"?Yh°–ÖÞ®?ïöŸ´ï>?8';'"•?RÀ–7Lú?8';'"•?ïøØZPP?LåuG똃?LŸ‹%'×?LåuG똃?ﺒ 8\?†AïŒàç?[wþqé?†AïŒàç?ïÚ«U¿á=?zµg㹂S?rªU)®I\?zµg㹂S?ïè
	2¢?TQ"ñ:Æ?gõö¹E¶Œ?TQ"ñ:ÆAGN4FGL J2249.4-1300¿ïI²¦4ÀMužèóÀ9<äw
}—À:ô؄ô@ OÏë1@ðúÄV܆?¼^z‰³ób¿¡UWv'Ù?ꋾßK@@½àJÙ?íÊt}€^_¿íz	ç	Žõ¿ÅÄyÇÑ¿é4mÙw¿åCå~*¨¿±ó¸žík~AGNbllRBS 1899?ïào"Àõ\?ƒÝ•TŠ?ok¤}?ƒÝ•TŠ?ïðd÷¦j8?c$¶`¬??_6"ï'?c$¶`¬??ì‹
°þÌ5?¨K Kæ7¡?»§'x	ž\?¨K Kæ7¡?ïÿ¼µõ½(>ójØV@ò6?҈ɮÙã>ójØV@ò6?ïÕ²Ñ4æ?yɁ"³=ï?u&ûviLú?yɁ"³=ï?ï±µÑwp>?ˆ#ò•·¡g?ƒ'‹"
Š¢?ˆ#ò•·¡g?íî[Ù"N<?¥½–Ó/<?°!6§ ?¥½–Ó/<?ïÿ]heïô?WÂöT'u?RòdX'A?WÂöT'uAGN4FGL J2249.7-5944?è~•CÀI§Ž\NµpÀ:ãÝéTÃÀ<µ&o<Ï@"W'
3D@M++ý´Ì?ƆîFD2	¿Ã~'Î?Çåóö@áÐj?¿ïñüÂ2êä?îAw^o¿ãP¸7åŝ~*¨J¿Äs6X¡U¿ïÿG©ýdAGNbcu3FGL J2249.3-5943SUMSS J224938-594421?ïþ€"û?!ŠRhH²"?.þåc•Ì?!ŠRhH²"?ïöò'Ç,?TqöÙ5ôØ?RÜ5.ºÅ?TqöÙ5ôØ?ïëx÷•ª?Z™Xm3?d‡ˆŸ?Z™Xm3?ïþÍ¥¥Ó?Ü ¼HÙu?#.øpQ'=?Ü ¼HÙu?ïû(k\?@₩]|?C‹_G9D?@₩]|?ïÖÚ߬o×?€5©›*Ì?t'3fü8?€5©›*Ì?ïÝS`áR|?vâ&–Ùt?qVO1è?vâ&–Ùt?ïûÂC9™?<ü¹i©}?CÄ÷`€]Ö?<ü¹i©}AGN4FGL J2249.9+0452?íekb‹ÀGJiߗª¬À;;m"XÀ<‰U>öµÔ@ÔBŒíd@£ÿYçÓ?ÁÉÓގ쿦ÆcÉuw?ãkD´e@¿o`
+Ó?ïÿQº÷k¿àšPCrŠ¿ãkâ§)¥¿è»F'‹ˆ¿àñÈ.Ø[¿††="«»RAGNbcuWISEA J225007.35+045617.3?ïþt'#?+ÓöeM?/ï¿"‰?+ÓöeM?ïícŒ;b?hك^Ú®õ?bœø±•~?hك^Ú®õ?ïñ:MÑ<?hzŠ"+´ì?]‹ÍæéK?hzŠ"+´ì?ïü<œ=Õ?"l»Ó7?>ÍEè?"l»Ó7?ïücž,s?:῅ÀÁR??¼áùˆ¸?:῅ÀÁR?ï§Ú%6+œ?‹E»˜ieA?†	vµä´è?‹E»˜ieA?ïâkÉÛ3?xV!Jœ?mä"Yà¼Y?xV!Jœ?ïî7Rý}ð?QúÒEQ?aÈ­C¸?QúÒEQAGN4FGL J2250.0-1250¿ï~Dž)ÀM:'£SÀ7`@ÒX'	À:oîÑ"2@ÎmÚÎî@Ìy1D?šw'ç+{a?Á+±I8®@*ç'Jð¿@!¥r6ð¿Å±Œ)™q¿Ò|	°ÛU¿åÁ£¾¶‰"¿äœÂä¾®¿ç€q¿àÖ¿ïÿôA…ÜMAGNbcuPKS 2247-131?ï`3
]?æ?¨°µ¿?"ùž¹m<?¨°µ¿?îîVb•Õ?µoEâÓ?¡š²‰°?µoEâÓ?鼪ù…?®þ7cO¢Ù?É
W¿¸ë?®þ7cO¢Ù?ïܼo˜¥d?ƒ'lCÝ?q¡È!j?ƒ'lCÝ?î×Vͅô?¦9⫯'k?¢Š"+[	?¦9⫯'k?ëTÖRv^E?ÍtÞ4—ü?¬¦¶&†ì?ÍtÞ4—ü?ì::k‹¿;?ªC)Êy—c?¾.,£¢%?ªC)Êy—c?ìªçû"ù­?½ˆnŽ~˜?º¨À#Ø2˜?½ˆnŽ~˜AGN4FGL J2250.0+3825¿äÂ|s¼À2Ô8ÑØ¥À9uTáä·À;ð/Þí@!dèŒñÀ?ûi¥ë·sŸ?®ôMS?'¡Ö\¡Q?ä?O™›G@
}ÙªUÔs¿ìô±d "?ǔ$9Æ_¿Ûguû.ßç¿Ó5dæ´¿âÒÐ¦¿´¸¨ÓsZAGNbll3FGL J2250.1+3825B3 2247+381?ïÿ,ÅÇ?
éUÕ¬>?j@y?
éUÕ¬>?ïñ¨ê¢ÿ'?cÍôU'?\®*dËcC?cÍôU'?ïôaÂtÔ?aõ'	–]?W<|FÈGt?aõ'	–]?ïú¢š8Ü?3ŒíÉõ·µ?Eu—¹Ÿ
l?3ŒíÉõ·µ?ïþ _d=? áÕçþÇÙ?%ú¢0? áÕçþÇÙ?ïǽž±†u?…±«¼ºcœ?|!0'Ÿu?…±«¼ºcœ?ïïÄ
‹ƒ×?rnyFéˆ?`;ò'¸¸›?rnyFéˆ?ïöi–ª?HbX.°ð?RÅ.0‰œŒ?HbX.°ðAGN4FGL J2250.4-4206¿Ôð] šÀN–HƒýP"À:"ë=ÑçÀ<æšÔ,=@ñ¾1""@¨Ú!I%ä?³ö¢3F(ƒ?qJB¤Œ´?À"z~K_z@"`d\?îE ˆ¡#Ò¿ã
AQ®ô¿ãL¦ló"¿à‹,žÄ{Å¿ãb¼ÃjM|¿Óð
H´ÐAGNbll3FGL J2250.3-4206PMN J2250-4206?ïþúgBb?ã·ý¾I®? YŒ¼_ª?ã·ý¾I®?ïö~΀ðÅ?Z1$HTp?Sb˜jf?Z1$HTp?ïø-¸H?A"ô$ÜÀ?OKÑÅxÛ?A"ô$ÜÀ?ïÿ7Ÿߨ?ôž'…`?í3À|?ôž'…`?ïÿ
På²?&v¥¢?]ìÔ>Ý?&v¥¢?ïÜ;/+Ð?~©D·?Ì?qâh^Èì"?~©D·?Ì?ïø2>Ÿ*±?\ühD?O7båº!?\ühD?ïþž"Jí\?ÇBÍ{?&Í\ëž?ÇBÍ{AGN4FGL J2250.4+1748? ?²©ÕÀB*ù‡?úÂÀ9ÿI¯vz±À;ü3Â¥@pªEä;@HPïܜ?¶×(˜¿ˆ"¿Ã'~Ó?ÅBÔ{lÝÏ@P",P¿ç%=Ì4¿ëË·XÇAs¿â.LC¥q>¿êaÞËÒÒ¿â£Ó¯?¿ïó¬ÐDÑAGNbll3FGL J2250.3+174787GB 224805.0+173330?ïýôOÑ,6?&kPWçc?0]'ª{Qx?&kPWçc?ïîÖ w]ž?bŠ°Ü 
Ò?a)߈¢a¥?bŠ°Ü 
Ò?ïáDIl@×?q×DVew1?n»¶mC‰?q×DVew1?ïúæg}"?1N/ç[2?EÀg:¤Gg?1N/ç[2?ï÷³.&j3?NÂ,	ò?P™£õ$9?NÂ,	ò?ï¸ß­Øžp?…Ž&éÓã?È—îÉú?…Ž&éÓã?ï¸ÒåÂ/?'ó%š¤÷"?ËF±0ŒT?'ó%š¤÷"?ïÖ»IRëq?iÑ8BlÜ)?t¢[b8ó©?iÑ8BlÜ)AGN4FGL J2250.7-2806?È#ÇXLOíÀO¨×ƒßóñÀ8{cRµ¯zÀ;™kŸ‹K@#ëÀ š@cTÁ"tŸ?¤õç"c'0?¸abEšh÷@ô‹"'Å@­ñâÝûŒ¾>êw¿ÓÜ#…}ƒ¿â¨½¯"˜¿âo–[ ¸¿ç+úŸ˜â¿ç+Kb©îQAGNbll3FGL J2250.7-2806PMN J2250-2806?ïûOŠ4l?@k3þl?BÁÖ1Í?@k3þl?ïéýúŸÌ?rÀΘP-?fá?kŠ?rÀΘP-?ï®VOBŒ?…l/vë8?"jl5UrÞ?…l/vë8?ïÿHfð½?=±Å4•«?ó1Í9†?=±Å4•«?ïü![šZŠ?;HÒӚ؁?>õ$+(jn?;HÒӚ؁?¬/(?´_%{ü?ˆÜð%b'?´_%{ü?ï¶|I/Q…?ˆ›|(⥼?'`í¿ÚJ¸?ˆ›|(⥼?ïþs]šº×?#a‡<é?(Ê%v8  ?#a‡<éAGN4FGL J2251.2+5550?ï'ñžW2À	MÔº.À:·¶'Τ=À<ž¡@W@´n œ˜'?ø­ä	)tn?Ք#c‡?â5ð²…"ê@z&3pp@"u€4ì?ï·²­fÖ?ïû"€«1¿ã¢à՘Mi¿Ô×DÈ¿éeã>~?÷¿ïÿ
Çhß½AGNbcu87GB 224837.7+553415?ïú=孈(?ERÖgkÝ?GiÀž­?ERÖgkÝ?ïå6ªOä?r¹çÊ®O?jÉU" ø|?r¹çÊ®O?ïŸ	VQ,?'tþAÐ
?œìÓ~?'tþAÐ
?ïÂÌý¸ìµ?e"),:?~™e¼?e"),:?ïò}õ½öŠ?`L©¨çµ?[¡L½?`L©¨çµ?ï.'~Ô,¤?®¾-×'š?š-Ð,Y£€?®¾-×'š?¢Wz³?›S†¢·s¡?§·EڈTÖ?›S†¢·s¡?`ì¬?"Ô,ö)Ó¾?ŸçÏM(Ô?"Ô,ö)Ó¾AGN4FGL J2251.5-4928?Êõ6SÀLù¸Që…À9ÂXr‡ÜÙÀ<;€kË*5@ ÛçœÜÅ?û½.äïÙA?´$í ,ì?º—ën£w@QJZ—%K@•#"™Þ?ïØÜx5?ÓÇ3{¨ø¿ÜÌÜÝ;/¿Ñà¤.Èë¿ß
0eMŒ¦¿äâO §)ûAGNbll3FGL J2251.5-4928SUMSS J225128-492912?ïÿr²5X?ÏÙ3I5'?±¥«d¢?ÏÙ3I5'?ïõ"}ê«I?[mOÂíœ?Tת®U?[mOÂíœ?ïð˜k=³?bt]/ë?^Ï)$dÙá?bt]/ë?ïþ¤ÝçÉ ?N@_dp>?%²"ðoµW?N@_dp>?ïÿ5Ë?­±Ó¾nw?9E0""Ó?­±Ó¾nw?ïÛDôž}?u]ü$få?r]…•vak?u]ü$få?ïæ
»EÖ?t\ìþ%<?iòế?t\ìþ%<?ïýÎÜ`Wr?$ˎƒ×p:?1‰œRôÄ?$ˎƒ×p:AGN4FGL J2251.7-3208¿âÏSÿuZÀOͳÐ|"¶À;6ªw7oÀ<­[.ú¿N@!V\îm†k?üy0ˆ^ó?ÆÔÏ»¼Ë?g"õƒá\¸?ŠÎ¥rž`±@Sõ.jÌ}?ïQ8×·âZ¿ë©Åá¡A¿Ôìò»ÈC¿àUçÈѕ‰¿æ¶b!Z?àU¹pޏAGNbcu1RXS J225146.9-320614?ïýÝT'Ê?-»m•…Ñ?1ÓT}2?-»m•…Ñ?ïìƒåŽuà?l'ÄŒR±m?c|¥Ä/z?l'ÄŒR±m?ïß}3åé1?{šnåh¶?pAf	›Ë}?{šnåh¶?ïùi'¥?¦?6‡µ5?JY¹ZTO?6‡µ5?ïüü F~?>¼-.¤@??¸Äo®«?>¼-.¤@?ï Y‡ìy?.#F.¢%?‡éž;UEÌ?.#F.¢%?ïڏB
?{¼X®hmÞ?r¸7ÞKvâ?{¼X®hmÞ?ïíijQØe?U$#þ01?b–•"ìK^?U$#þ01AGN4FGL J2252.0+4031?ä'ó°nüÀ0ã"[tšÝÀ9>Ëò²9¤À<	z‡…›@À'Ÿ:'@Ñ"2w?¯¨Ž¡ebR?¤9¯¤A?ôü…×Dö@	\'»Ô¬ë?ÒÞ&[´[½¿ÓSˆþ–É[¿á–¥ÞÌS«¿Ü|—UG¿â§ýª»*
¿â¡·ªü˜lAGNbll3FGL J2251.9+4031MG4 J225201+4030?ïþC0¦Ø? µ™ª`'?+Í›-¯? µ™ª`'?ïñm`U«-?bººZí'?]%>ü³¥ú?bººZí'?ï÷°è¸?@J†…'†?PŸÉ—4ÐÇ?@J†…'†?ïéç[)­Š?Q5˜)?f¤ßñ^Q?Q5˜)?ïý<Z"
R?(@†
x?6*VI'?(@†
x?ï¿eNÊy?Š›;ó/¾Þ?€&¬N"Ü?Š›;ó/¾Þ?ïøýR"9ê?Xß'þVɚ?L
¶þ¬«?Xß'þVɚ?ï̖ì–×?f"í}·ß×?y´‰»ÔL¶?f"í}·ß×AGN4FGL J2252.6+1245¿˜Ic'M¦ÀDf¸w«À;<Ÿ1‰À<œ׊•ñ@ lià™]?þúEዠ³?Ê£âëE?½g³¶Ñ?ò"ßq?@@Î*oë¿ïÿýFKê?ïû×ómK?äÜ7£~ö¿çOHÿ΂¿â•Oçžà?µüé=ÝÜAGNbll2MASS J22523220+1245109?ïþÚÕ4`–?!8?=­á?"R©d¾%?!8?=­á?ïå(£Y®?ozò±+?jë×?əê?ozò±+?ïÙ+âß?wôä½°?sjͬ5?wôä½°?ïàÚ§<*º?XiÓ4CIC?o%X«T?XiÓ4CIC?ïþK
ñ?$°‰¬tS?+O`Í4¥ž?$°‰¬tS?å"ÿ"?'7"%L?ŒÚ†žÀ?'7"%L?ïÎLñ9m?€@‡b•
'?xهWç	q?€@‡b•
'?ïšP3|·¿?z¿ñ"ÉՅ?‰kó I?z¿ñ"ÉՅAGN4FGL J2253.2-1232¿º•ø5—w½ÀM]Ñ_ÄÖÀ9ß=ÍÀè"À;À®J*Æ@*ߊ¿¥@ÚøßzN?Ô€"ØA?á©é"mé@›ç¢;(Ë@à{/Ì ¿á×xø9b¿æ=¸È3
¿å¢Z¾ž
¿ìÿ atd+¿ãHY€NïÒ¿ÐFPܼYAGNbcu3FGL J2253.1-1237TXS 2250-127?ïøÇ&šž|?Q®ÌŒƒ,*?LãdùdœH?Q®ÌŒƒ,*?ïìš{§ýF?f=Àé¶ZÏ?ce"<…ÚZ?f=Àé¶ZÏ?îjÁ~SÜ»?™ãDz¢?©SèæMU?™ãDz¢?ïóîžà?E¦ü&éÝ?YÈ"Ôx`7?E¦ü&éÝ?ïêz"ü!?m쳁v´?e…îmc·1?m쳁v´?Ewò?‹˜´<>;þ?‡V.Áџ"?‹˜´<>;þ?í2W€šo-?¤ÅóQ·Pæ?¶mCüäT™?¤ÅóQ·Pæ?ï­×Ϧ?x-:í²
­?"¼Ê¬z€?x-:í²
­AGN4FGL J2253.3+3233¿°3;£ÿüÀ8	"‰a=À;-Ëë%À<fÙþ
·y@ 4ÓÇ=@o³·RE?ƒìÁ´À¼¿€Ã@ö¯
8?¹!˜¿/@g‡ÒœÅs?ïù]¹ïzw¿ßmµ»
\µ¿à²ž­›¯¿èòÂ?U*¿àq¹KÈ˿ے¤²ÒOÄAGNbcuCRATES J225312+323615?ïþ+\­³‹?#°,IÌ?-J2%QÎk?#°,IÌ?ïñ' ï?b'¦îÝ<?]ÒÝÁ¿c?b'¦îÝ<?ïíyí¤*9?`Š`ñ¦XÁ?b†|Ò"?`Š`ñ¦XÁ?ïùßГ3'?*÷»ƒ´ƒ5?H€½PÉ÷?*÷»ƒ´ƒ5?ïúϓjoN?@ɽåÄ?DÁ²Ì'?@ɽåÄ?ïÁ"æ4/?ˆƒWÍl;?5Œî×3ç?ˆƒWÍl;?ïÓ÷ŠªWF?z¾÷µ£L`?v:ÉÀØí?z¾÷µ£L`?ïãß°K¯"?XÑ·öI?l O¸pe–?XÑ·öIAGN4FGL J2253.7+1405¿ïZ­åDØÀCîWûi˜JÀ:Îb«ÆÂÈÀ<v²¹%P@ ¥‡4è&?þLhĸ*?ÇläDb°y?À|êŒP[?õºÂùå3Ì@—dÌÞ?'?îϾB'¿íè¡^ßßN¿¸\2ZñQ¿âHMv«X¿Ý&-;L‡B¿ÙvÞ¸1µAGNbll3FGL J2254.0+1403NVSS J225354+140439?ïÿRú•/?
ôÓ¼àåH? ¿ÉºZÇ?
ôÓ¼àåH?ï뎓x«?hkðºÏá‹?dqlXµ¥?hkðºÏá‹?ïøûýš}£?<ïDÃX:0?L	ª`¾O?<ïDÃX:0?ïöøáÂl?5·Pf…R2?R<%ñ']?5·Pf…R2?ïþŸ‹Ý)¢?"û½æòUŸ?&?¿ÜÜ?"û½æòUŸ?鸞'ÿn?Íz]}Þ?†×Û9EG½?Íz]}Þ?ïùšl—Õ?TJ.{>N?I–LóñN?TJ.{>N?ïäðK›Î—?[^´óg˜?k´GT±=?[^´óg˜AGN4FGL J2253.9+1609¿Ñeht³†*ÀC©~+VÀ4ºaŸWH¼À:›²xŽ@ˇįó@K̼ܔÁ?|gÈ_V‡?¹¬‹cË×Y@C‡~|â@%ᖏùÞ¿Ìú'WÛß¿â3ÂÚۃI¿æÎÇxÏõ¿æÊֈ7q†¿ëa#0†°‰¿ìVB+ÐAGNFSRQ3FGL J2254.0+16083C 454.3?í$	W .?ŌN+Í
?¶ßß´g•?ŌN+Í
?¯Žžy3dà?½@93°å?î_B?½@93°å?écÓ4¸Ö?°|J€ç"?Êp³ã-ª?°|J€ç">÷¿÷¢Åôd?¹Œ	Y?ïÿÐß´0?¹Œ	Y?íPΰbïö?¹4'§
ɸ?µyŠ|è€T?¹4'§
ɸ?¼ø‹šè?®°Òñ)"Ž?ï{'W 	?®°Òñ)"Ž?ìäéøgì_?©æӂ€?¸Ø°;Ï
?©æӂ€>k¯ñƪbþ>žâ"ð_(•?ïÿÿä,§>žâ"ð_(•MIXED4FGL J2254.2+4305?èJ€ß/ó/À-'L¾´À:‹"XÖÀ<Áh¼P@ª>0'D@^e'
?»öùŠp¿p7}¡"°?­xŽÃ8	Ã?â%ébs¿áò_-¿åcŽDÑÁ(¿éÿ½Ñb^¿âíŒM€¼¿ïûS]u&?ï¸d*LåAGNbcu3FGL J2254.6+4253B3 2251+428?ï²Lœ¡ó?±
µµñ—?ƒlÙ/yE?±
µµñ—?ï7~blÂÝ?¨Ü"v1D"?™3·U?¨Ü"v1D"?îÞΓ1±º?–0b»w?¢Μ²]?–0b»w?îÚ$±À?'™‡6PÛ ?¢]´ó›«?'™‡6PÛ ?ïÒ4ñë†?•ÓÎÒî?vå‡2«¥=?•ÓÎÒî?æšU@Ï(?Ñ-I•±hÔ?ÒËU~a¯È?Ñ-I•±hÔ?î'Ü: \N?œK+‹?§Ò<Sf†&?œK+‹?ãÎ'=?ÃufºÛCï?ØcÁ±÷Ņ?ÃufºÛCïAGN4FGL J2254.8-2725?í²¦5^[«ÀP	ÿÖ"îÀ:D¶4‹À<,ü<& ü@ ×0;Üúí?ÿò‹ÿH?ÀœÒ^18²?:燎)N?ÐɒZ¶@·{ý+?éý+4¾y¿çª|?ì¿à»²}ì¿ÜP'¤_›F¿â"?_'`¿ÅÑûÆ_uAGNbllNVSS J225453-272509?ïþ,±
ÿr? îàC˜àæ?-4î×w…Â? îàC˜àæ?ïð;!œ»k?eàPEßQ?_‰¼ŒÏºö?eàPEßQ?ïõ5'Ì÷?IÎÙ¡z't?U•þêä2m?IÎÙ¡z't?ïþxiÚJu?Þj)½@'?(ydzS~?Þj)½@'?ïýI§òU{?08áeD®?5²¿jñˆì?08áeD®?ﳦf—ÊÉ?ˆcÖhM"?ƒf[ÅÕ?ˆcÖhM"?ïòER*Ö?h©R¸¡T?[Ñu|¦"+?h©R¸¡T?ïüû®*y?,6¿t,2?8"ŽZÙ7è?,6¿t,2AGN4FGL J2255.2+2411¿ë·MYؗÀ?ˆ;`(^ÄÀ93´±M†À<IF"@n[4Ùü`@Ûª€qªg?¨àA¸uí¿Uäa`d'?±¯Û @Ê! c¸6¿áþ3a¬Bi¿áNË?.¿â<8*ù¿áŸà¥Ç¥F¿àßÕó¼ûž¿à&JLTliAGNbll3FGL J2255.1+2411MG3 J225517+2409?ïþCÚË=+?ËDMî
¥?+ÂPö
ñû?ËDMî
¥?ïò%Î_É?^|àkß"ð?[´c¦˜Ý"?^|àkß"ð?ïøþèd?Txè?OÜgÎø?Txè?ïùÊÆ&.W?9éim?HÔçf-+W?9éim?ïü2Î^rQ?4§ÞÉwB?>iŽ¥r'¡?4§ÞÉwB?ïʄ<Ýxc?~-(…É?z½á£Ñ²a?~-(…É?ïõ´öIüV?a¦pÒ°þn?T–HKd(?a¦pÒ°þn?ïó!ÅÍ$?Pñ¿°Û=?Y¼t©¹ç?Pñ¿°Û=AGN4FGL J2256.0-2740?ï«Ékˆ(ÀPýŸÓo~À9<çƒ1xHÀ;Uù†i;-@åBÕ<²ä@¡…÷%f?´f~«<ë?'Ÿ˜6B1S?ÚÔ֜?@	ðÖ. Qo¿ÝŒZ@é)O¿éÃÌÞj"¿êˆì9ò¿êŸ<¦y{í¿ïÿtN†v?ÇÙ府mAGNfsrqPKS 2253-278?ïú¶U£0Ø?XéX¨öt_?E&©óTtˆ?XéX¨öt_?ïî†ÛH]?psÉ^*?ay$€©7æ?psÉ^*?îü©žÊ[?•þÖÊwª? 5fÉëÓ?•þÖÊwª?ïúVS&v??8yQ?ýÚü?F¦´x{º?8yQ?ýÚü?ïõh칸?`I,×ìëò?Uÿ."€µ?`I,×ìëò?ᄔÐ?¨ÁãaO*?‰"‹ø"?¨ÁãaO*?ï&ßx~Ÿv?•q`l0½©?›$ì¼uI?•q`l0½©?ïÓØ£Uì,?mÈԚ¡p?v®Z‰Iþ?mÈԚ¡pAGN4FGL J2256.4-7119?ã*®JÖÀE~p\‰mÒÀ;~à^zÛÀ<âòŒyöf@""'y´¤?ó§®ë:v?ÓmJ[BñÂ?Ûpmü1ê3@ ÀŸ—à\@õƒÈ!{?ïû¼PíX¿æá¨&$W¿ïÿïXz?ïÿÝ/ñ_S¿ÖA9†3‹H¿Åüº¦.¨_AGNbcuPMN J2256-7115?ïûŸs"a?:|Kn)?A'3HLá?:|Kn)?ïóÞSÝͦ?\ÃFhP•©?XCWô­ÄM?\ÃFhP•©?ï½=}Žöþ?zŽCKŀ?€° –ôu?zŽCKŀ?ïû1žBv?;q˜ ¾?=?C;±ªó?;q˜ ¾?=?ïûU…%]?FLך"·4?B©‰æ^?FLך"·4?ïΉܞb<?ƒ¼ÖR?x»Ò¡õ?ƒ¼ÖR?謁l,y?"ô¥Û{¤,?…På .¹?"ô¥Û{¤,?ïéð¯?d\‡ïeè?fpíeâ?d\‡ïeèAGN4FGL J2256.6-2011¿è¬'ðˆÞÀOr" ٔ[À9cÑû	öúÀ<1¾Ûrþ@Ìâ'q	@À5¤'?¬˜ßàOáj?šgà9B?íñg™T@D
ájÿà,RÚš¿ßECÁu֜¿ãy î?
¿ÜEíhMÇ¿æƒ_—±¿äiM š)aAGNbll3FGL J2256.7-2011PKS 2254-204?ïô43Î9?XÏ`L/QQ?W—ÑqOC?XÏ`L/QQ?ïëL3¬?iÊr#d?dÿ´1F³<?iÊr#d?ïěD-p??~
æï%ýÂ?}²]ØÉÀ^?~
æï%ýÂ?ïÉËgG?iæž<Ô?{@l¨ÍÒ?iæž<Ô?ïÐÿT'0?q²ø2|º?w€U½,3û?q²ø2|º?ïO>4KÀ?'I,…Ve?‹ì0yÌH
?'I,…Ve?ï¥'ë2ò?‰?Z'y˜%?†¶<Rñ³o?‰?Z'y˜%?ïC'O$Uu?w|‰"n?—›½ƒh?w|‰"nAGN4FGL J2256.7+1307¿ïY úO֜ÀDˆŠÅÁ@À;~d^NÀ<5·qñµ@ S‡QŸ¯?þ+£!h0?ÐKÍ=µî?Á•Æü(Z?ò-žž¼J@žx±A«ò¿ÞÁÍ_™Ã‹¿ÎÀ¸Azsº¿Ø«hC`Qú¿Üö)RáP¿àVÎþÖ4U¿ïÿóÀ¬ƒAGNbllNVSS J225624+130541?ïþ´<pJ?ˆ»ißû?$¼A…¢"?ˆ»ißû?ïèÈa5؈?l\¡€•ª?g7Ÿø?l\¡€•ª?ïð¿÷†?[}ՋgÈ«?^€"v¯?[}ՋgÈ«?ïõ˜¡³)Ê?8G´üL?Tμ÷!Ì?8G´üL?ïý¼"w|?0‰ٗÎÐ?2åݼïº?0‰ٗÎÐ??2ËMS—m?‰¹ønB&6?2ËMS—m?ïb9?lG‡'SÔ¼?ap]Ý?."?lG‡'SÔ¼?ïÙA¥;ä2?b–l¨q¼?s_-H ËB?b–l¨q¼AGN4FGL J2257.5+0748?ÜS¦‡áÚÀF¿ŒâÑñÐÀ:֟vRl´À<n¡¾+IZ@X>A¯!ì@'ìCŠ™L?Я¢šÛ¹?¾1ì'9ÿ?æÕL}‡\@«QȽ/¿ç8"Üû¿çwk§^¿ÓàŽ€`ãp¿ç͑¸ú‡ñ¿ïû5`4>?¿¦Þüz9'AGNbllOY 91?ïû(wÃ[	?@H§"â±Ò?C^!Æȇf?@H§"â±Ò?ïìõ2ëú?cÄP]Ú¶?c
Î3­î?cÄP]Ú¶?ï"O£?…Çýùù'_?Œ»óŒß_?…Çýùù'_?ïóWÁï	t?C7þºÅ!š?YP{ø±È‰?C7þºÅ!š?ïôkô?V˜jÿ*'©?W(yUA?V˜jÿ*'©?ï¢Õ"íÑæ?‹H"Ô·-?‡J·Aêq?‹H"Ô·-?ïŽ4£(l?Œtå¼$6€?Œz²×5äò?Œtå¼$6€?ï¾tÆaµ?q$€p^%?€xbÐÏLÄ?q$€p^%AGN4FGL J2258.1-2759?æçüýRaÞÀP;0"'À8=RpæÀ;Sß'Bd)@ ÔûðPà@L…0aÈ?¡€Å?î?ÉVEÜÙ	q@#–žš@¼à€ø¿µ¾!Á¿ÛFËÿ€¿åM1:Æ¥¿è(bTˆîQ¿ëOý¤-f¿í
òl™†NAGNfsrq3FGL J2258.0-2759PKS 2255-282?ì_é%·¹Y?ÈÞÇbÌö5?½¶ÒB57?ÈÞÇbÌö5?ï´à¥zV?™óƒ³!Æ?'ÇÖ¤Úù?™óƒ³!Æ?èÂk©¶?²cl> ,?Ì÷úQY'Ó?²cl> ,?ïéIíßÁò?i"Ö3õÆ+?f¶H…Ë?i"Ö3õÆ+?éfŸöø;Þ?À›7òhEl?Êe€$‰?À›7òhEl?îɤ—à˜?³+vÿ¥b?£e¶—'?³+vÿ¥b?æëL'þð‹?´íÐá™"?Ò)fÜé?´íÐá™"?ï-›âÓ?"8Ÿ©ŠÍ?šL§9??"8Ÿ©ŠÍAGN4FGL J2258.3-3643¿æ1ÑuöH¿ÀP*0U2aÀ:–…`ýpÚÀ<¥šàÁvW@V¯ÂÐʈ@š"ù$D?ÀlrYŽ¼œ?£tå㧸I?ãm­¸4T@	9Yèԕ¿ï`ƒ-FŠ(?ïòI~N9Ÿ¿Ü)ªu[Í¿éŸKT'(Œ?ª›ÈüfK¿èW'[åYAGNbll3FGL J2258.2-3645MRSS 406-025483?ïúBÓS?P)C¡‡ËC?Fô³·Ú¡?P)C¡‡ËC?ïëLš† ?pR4®‡˜?d³f7ž?pR4®‡˜?ï´[èï?ƒ—3¦‰5Û?'é,g,V?ƒ—3¦‰5Û?ïþ'?ÆûŽ?ÔÎpë+?'Üè=#Ì?ÔÎpë+?ïðgã'à‰?d¯o&ýèr?_09Dv|á?d¯o&ýèr?ïq¢ú7áe?›oÊók¸"?'Ë ²$›d?›oÊók¸"?ï¸4b:æ9?"9Aÿ.?òçjg9æ?"9Aÿ.?ïûJùùUÂ?=àƔÀÚ}?BÔvHvc?=àƔÀÚ}AGN4FGL J2258.4-5524¿ÜçCÛ÷âûÀK;Oag#À:aƒ3%Ç:À<¯
@Ë¢*@ya¸âÔ@(a´Oþ?²ÓÁž‡Á¿¬§i¢Q?úPŒû%¥¬?ÿÐÈLŠr4?ÄÍÀ"!¿çÓ²ßæ¯ø¿ãÔ%¼R+F¿à"ØÅ0 ¿Û]:É)ª¿æAž¥AGNbll3FGL J2258.3-5526PMN J2258-5526?ïúö°˜[#?3sªo'Ï?D%=?V?3sªo'Ï?ïîyçò¤?fD	™*¹µ?a†	›õ?fD	™*¹µ?ïé0×Òÿ?n´ûU'y?fÏ'øÆë?n´ûU'y?ïñŒŠ<"k?C5š 8œå?\æëò*ú?C5š 8œå?ïê,4Ø?\{Ùfw|
?eÓã/¥`(?\{Ùfw|
?﵃{[QF?pÏWý?'Ÿ!:Ä~?pÏWý?ïÆÁ4_¥y?'=!iù@8?|ŸeÒìóE?'=!iù@8?¼5rJ?|uVŸn!Ë?‹ØëÄ5"?|uVŸn!ËAGN4FGL J2258.5-8247?ä̀
É©úÀ@¶ YžØÀ9Г¯tÍ1À<4‹ƒVa6@*wB+ɇ@¥ ¶Xí?»]7ÄB?ç-@÷Ý@A¶Ô=—@:«C:<g¿à.'à¿ÙÈõ<WŸ#¿Ú!(¤c÷÷¿Ý{ñ½òêC¿éEÚÍa¿ãdeጢAGNbcu3FGL J2258.1-8248PMN J2258-8246?î=

¹ÀÅ?Ë\)2î?¬/_"¬%®?Ë\)2î?ïôÃ:Ê"Æ?Vދ›±?VyŠ'DË?Vދ›±?ïËtœxàÖ?zpƙÞ_0?zE±ÜLÄÄ?zpƙÞ_0?ïï…ä°ï!?H›XæN¤H?`zƒJï?H›XæN¤H?ï̍½ èv?u#[T²…^?y¹!>ªì?u#[T²…^?ïÓ ò1û?ƒwˆ§uќ?v/†ûd>^?ƒwˆ§uќ?¹³s? ±··EÒ?§¦—ÔdÊ? ±··EÒ?/Uà?oþnÅuA?€Ü*´CÉð?oþnÅuAAGN4FGL J2259.7-3549?íõ"À³SÀP05~gÀ:zj]këáÀ<•ýÉÄÛ@ì&.6Ÿ@ewmÏ?»¤ðñ4‹¿"ž/aê›?ØñOƒJø¢@žëq}›·?—¿¸€ÿ2¿¿èWï«&\¿æ>´`šI˜¿×wR|¤–M¿í þG™ſĒ©ei'>AGNfsrq3FGL J2300.1-3547NVSS J225941-354846?ï⦛é2½?mbNâºÂƒ?mYdZ%›?mbNâºÂƒ?ïéæï#?p¬öXbrá?f÷½Xá?p¬öXbrá?ïoí㷏? m®=ÿ?''<©Ö2? m®=ÿ?ï÷:Í9î?;ý‰™A¶K?QŠe'édj?;ý‰™A¶K?ïÀ<Ð.ÅÕ?xÄΫf!$?á—Ö¿›?xÄΫf!$?ï{ˆ>®ð?—à'È!
?ŽývrT?—à'È!
?轢ux/?Š
cØ­Ûº?†\¢È`d@?Š
cØ­Ûº?ïÞó·-k?a'®–¹éé?p†$hˆ^B?a'®–¹ééAGN4FGL J2259.8-1552?íZHTâíÀNå‡?úÁÓÀ9ùqÆùgÀ<`9»°è@7/
.­@DJ9ßõž?º+œk[?ºÿ"JOY…@µ­é¿@b?Š.˜¿Ò¿žÁ÷‡¿ÜÂn$ïß¿ãbåþL À¿à®°³ ¬¿äŒñ_Ô&¿é¨eå7&ÞAGNbcu3FGL J2259.9-1553GALEXASC J225957.26-155332.5?ïþrÏÞ؜?®
3yJÀ?(Ó…¹zœ?®
3yJÀ?ïîK]ݑý?qnyâÇnj?a´¢4Kú¾?qnyâÇnj?ïôXÿ'>?Iù®^foë?WNd‰åm?Iù®^foë?ïü	]̹×?'Êl†ü­??µíÁ]@?'Êl†ü­?ïü‹sçƒ?3DµúdÒ?;¤a+ú ~?3DµúdÒ?½Æ¨#?Ž¶<g¶?‡œÐ˜¤Ë(?Ž¶<g¶?ïéQÏoXA?q	{¹ê³ò?f®0Êa.a?q	{¹ê³ò?ïõf)ø?E·y÷Q¤?U3Â	…Pì?E·y÷Q¤AGN4FGL J2300.1+4053?è¡‹wå6À1=³(é-À;4½çXÀ<œIwBV½@":QŠŒ5ƒ?÷˜ƒ$"?Ó¶, ð;?Ñ5@Ԇ€?ú…dÃÎ÷I@õ˙Fª?ïpŽ• ¿ïúS] ;?íÒ ¶ÄLÌ¿¸úÕ^@Ó¿Ð9*ƒŒ<¿Ù?͚'AGNbll3FGL J2300.0+4053NVSS J230012+405224?ïý\""×?&"!ô43?5`àãûÎ?&"!ô43?ïïUP"±?e颦t§©?`ª°	I6?e颦t§©?ïé€3tª?XãFµhÑ~?fï±uý?XãFµhÑ~?ïí>óÁêW?PüÈ$µÙ¤?bÁ@ÕY ?PüÈ$µÙ¤?ïþb+ÌÀ?!=ÈéŸN?)ÝES'P?!=ÈéŸN?ﺩÑÙ?"ˆWÏdƒ?U‹Ë™Q»?"ˆWÏdƒ?ïï"¨'¯?kV>ÊnåB?`âlnÚ¨~?kV>ÊnåB?ïÞ-`¿?gºä¨Å¶J?péOêƒ?gºä¨Å¶JAGN4FGL J2300.3+3136¿ë4´döúžÀ9'ê>xâÀ9'üaåÎÀ;øV"ŒÂ@d?3F©]?ûÀ§$œ—?´(Ùþc´?Ãï$eü¸@cÈ}²³F@Qä&?ïæªY~?×êdbU4»¿Ôòñ#Ä*g¿Øj'ò"È¿áæïÃqÚ8¿èŠ.A±ÑAGNbll3FGL J2300.3+3136NVSS J230022+313703?ï™þnZ|?¤	²4´×Q?ŸìÀ.Å'?¤	²4´×Q?êá(¿;ê'?ÆjÀ{ŽIb?Ä{]U¹?ÆjÀ{ŽIb?íÞ·'kv=?ž³Öè¡Âò?±
FÃÈg?ž³Öè¡Âò?ì5TmX?›ŽS¡t?¾U\—Ÿ]B?›ŽS¡t?꺾E±¡3?»Áç–Ó?Åé9{2?»Áç–Ó?Ù´~±`á?Ò­ðŸP?ã%òÀ§O?Ò­ðŸP?ë Zd5Æ?­VD¾Íþ?Â~–o(é?­VD¾Íþ?áĊl%Ý?·óz¥Qw†?ÜvêÅ'´F?·óz¥Qw†MIXED4FGL J2300.7-2645¿å ³ÍnÖÀPWæšÔ,=À:ݲ"ý[
À<{k%@áöfÏÿ@i=¾§p?ØOsûÐE}?ÙNäH•@:ßdš@Næ¤g¢¿Ü÷K%˜?ý?ìԝ¡;#˜¿â~\&qƒÑ¿ä‡ä€G¸ü¿ïý~E€<ѿ䈴€ÈAGNfsrqPKS 2257-270?ï	o?^xù®/½X?`û]eU)0?^xù®/½X?ïìÕîVà?eßÜmÚq!?c*¿üŸð?eßÜmÚq!?îã Î8ª
?Ü<I-?¡Åó™x1?Ü<I-?ïðe'ÎEÀ?Iá'ê)$ú?_4Ú¨,¯a?Iá'ê)$ú?ïëg[ü!›?c¸y\Ðùø?d˜£ÿ¾Üˆ?c¸y\Ðùø?ï¢Å›ïÎô?ƒ>;䂂?‡N˜ý-
ý?ƒ>;䂂?îÒ8µºGË?—­&T­ E?¢Üt¦QK?—­&T­ E?ïÏÍó­%?l÷P?CÈé?x{˜÷%?l÷P?CÈéAGN4FGL J2300.8-0736¿³ïfX±"ÀLªt)ˆ<À;1²åšùìÀ<¢f®ŠÂf@ ÔÏj5þÀ?ÿ:o¸¿ß?Ã÷¤;Þþ¿§öO¨ó?äëûѝ&?û²{诿ì,¸Å®ËZ?'¿FÚãn'¿ã®ÊM–‹È¿ÖÛt/|ÅM¿åÛ;à€Þ¸?Å£3÷(kAGNbcu2MASS J23005469-0735438?ïþd.D‹?–ï0ø?)½@ƒ2?–ï0ø?ïå٥řI?pâæ¹?j&Z6G.Ò?pâæ¹?ïðé7Y?S5Ú×B?^-àJD}!?S5Ú×B?ïîÖ´¤"Q?I´ë,¹w?a)K/€¯"?I´ë,¹w?ïýo&ñ¯?-s1œ€>µ?4†ÎüŸ?-s1œ€>µ?ïti­SñÖ?–>íä?'rÊ\`ý<?–>íä?ïòSgl\?h&@Y(¹?[óXú-ˆB?h&@Y(¹?ï‰t¨žoA?w×ԝ
³?¢ÕßCg¡?w×ԝ
³AGN4FGL J2300.9+7108?Þ)¾í]ˆi@$XNaŒâÒÀ;B* dúVÀ<¡'~Ê
{@ íœøž·¼@g£Àd¾?Ö2%™È"?ÝMŸ$óÕO@0K!f'@F2"QÜ¿ï²BÝË!Ò?æ÷,Êx?ïÿ×ñÃý¿Ú°ïáú±b¿ê\Ö/Læ¿ÚgC›‹6TAGNbcu87GB 225907.3+705409?ïåÛ¾?fÇљœêù?j$Bg$?fÇљœêù?ï(;ÀËa¾?¥CÅ?šø‡èK–G?¥CÅ?îé*ÇK?"÷^"o?¡o¾Üw¤L?"÷^"o?íWaç.U†?ž&°Ã×°¬?µDðÈE!Ê?ž&°Ã×°¬?ï‹v€1`?‰±pŎ?"_ð8^W?‰±pŎ?í"í›Î?º±gìxd?³`—iÝw?º±gìxd?ìœ[l|ï?¦ñ@-Cdl?»$œ8ˆ?¦ñ@-Cdl?å¿-=Œ
Ñ?¾Ÿ|®7œ‹?ԁ¥"çä^?¾Ÿ|®7œ‹AGN4FGL J2301.0-0158¿ì¡ÉšïÀJÁ—¢H"ÄÀ9KþmuNÀ<͆00I@	('Ö¶@ˆ+輜?°ðZE›À?»{u·O¸@S;wG@¯ga8)¿¿8¦³³v¿á垪Ðy¿æ½}h5ž¿æ†yKD!¿éïj¼6|"¿ïÿîbHÊtAGNfsrqPKS B2258-022?ïý<b ¢ç?+ä^DjF ?6èîq7-?+ä^DjF ?ïîîؐOn?dÙs¢"¼Í?a'/ê]?dÙs¢"¼Í?ïäþca"?aäì
çš?kœ¿i9?aäì
çš?ïÿKH9ý?p~ÍÚã?–÷_Ï¥Å?p~ÍÚã?ïüèçh7*?3edz¦É?8¸Æù÷J?3edz¦É?豈à1¥â?ŠDHÏêõ?†ßÇð&ë"?ŠDHÏêõ?ï³*±¦Î?|ßþo<o?~¦jĹ<Ö?|ßþo<o?ïþx°¸;"?-ã md?(tömA†‡?-ã mdAGN4FGL J2302.8-1841¿Ñÿ‡"ßJ©ÀO×L`RPÀ:»¸/†ÖHÀ<¡Èê¿üÛ@ªòêí¿@ä"]?v8?ƶgZ­³?­1÷㕪æ?åÌÙAÐ/@]tWjÊú?ì!ÙzZ9¿ä¿'Bd(Ÿ¿àüö•óò¬¿áï;â"D¿æZUÖ¿ïÿo˜AGNrdgPKS 2300-18?ï÷'ödP?M;cÒq?PÜp=?M;cÒq?ïêÎ%΁ê?uRhtáèä?e1ÙòEFw?uRhtáèä?ïâӃí'F?i1"5E
|?m,{ð!¡Ì?i1"5E
|?ïæOev"õ?Pâ"*¶	V?i°šZBÑ?Pâ"*¶	V?ïæ,€Ê?dˁgÛpÓ?iÓ=Ac~~?dˁgÛpÓ?å/*v?'¸P¸c?Š'­V*}?'¸P¸c?ïÆéýpiÜ?à$ð[¼y?|‹U‰'?à$ð[¼y?ï­({
b?oهVß's?"µà~÷}?oهVß'sAGN4FGL J2304.3+0618?ì•ëÀGÙmã2iàÀ:¢iÿxÄÀ<`FS¡gÄ@¾
0•5@úxCÞ|"?Ï0Æ[ïj?ÍGÇêºÉj?øc×ZÅHt@
å+|…Œœ?ïþ~ÀÐ?H¿áî÷. &|¿è™¢¨áá¿æð(A<¶?¿ïÿ¿h`;ª?ïZZ¿i6ûAGNbcuPKS 2301+060?ïævÊÒF?¥ž	Ù²3O?i‰6ì)º?¥ž	Ù²3O?ïíÉò?i0!§:}?b6æÁ̅Ù?i0!§:}?ï¹¾v.Î?x•ƒ¸n_q?bw:<q?x•ƒ¸n_q?ïø¿'G]?7üÇÈþ?M»ò­»?7üÇÈþ?ïýЇ¹¿¡?1ÃFµ|œ?1{žÜü?1ÃFµ|œ?廊ÖDè	?Ž=?†ÕÊyѺ?Ž=?ï'×oVéµ?ˆÐ"šâw?J$‡"³?ˆÐ"šâw?ïÙìJk‰?bès"Ñ?s	ÚÕ:7ì?bès"ÑAGN4FGL J2304.6+3704?ïish}À5¤]AúvÀ9"n"2QŒÀ<XÓÖ¬@ TÐó"?ýpoiDg8?±—÷-š?}ÅmáC¢"?Íè¤CÁ Ê@
/¬G¿»¦æÿ(¿Ûl¢ Sr¿åï¤"^¤¦¿ÍEþâô¿ÔÑ{ˆ6šÇ¿Ýá/ÅÀiAGNbll3FGL J2304.6+37041RXS J230437.1+370506?ïÿ'üÁ?û7×I=?[B`j«?û7×I=?ïòï0yð\?b֜OȒp?Z!ŸlTW"?b֜OȒp?ïøvE£ð'?TFõ?W7Û?N&êjG?TFõ?W7Û?ïþíÁí~Q?
–µ©v>Y?!#ÞKԝø?
–µ©v>Y?ïþã+ͨ?wp;ânÞ?!ÍGEÌË?wp;ânÞ?ïÊØâ'£?"¦åZØÖ«?z"ŽëPR¡?"¦åZØÖ«?ïúYP0øy?O
Éí
?FšÀ5´íÖ?O
Éí
?ïþSWx¬?€Y`cêˆ?*ʎ•Æ'?€Y`cêˆAGN4FGL J2306.6-1105¿ÕÃÊOnþÀNMêhìSÀ;+š8ûÊÀ<¢RÃò2¸@ü%4ÂÕR@éĤà¹?Âìv¶?Ž¿œ«ÒèUûp?Ü}Y\'¨?þdÐTÖ×?îI±Y¤·?æ*¿ëò¸ࢿÙÅ» 'è¿ÈO8·×rB¿æ®"2Q‹äAGNbllRBS 1943?ïû7‰·¬Þ?=Õ oXæ*?C!Ú#¯(?=Õ oXæ*?ïå–<—àÝ?t{
¹G®ó?jiÏúšú?t{
¹G®ó?ïӒDf\?~È
	2?v6ÝÝÏR0?~È
	2?ïôXUgÌ©?DGþ$Ñá½?WOU›½7?DGþ$Ñá½?ïÕ}j§œ?ykõ9õ‰?uAqGìâ?ykõ9õ‰?ïsš=·?ž›¼‹€?'Ÿœ±ß³?ž›¼‹€?ïÒ#śÄÜ?}"Š¹:t?vîIzéô?}"Š¹:t?ïÀ•·6ãl?uJ÷
%?µ$pìáô?uJ÷
%AGN4FGL J2307.4-1206¿ï2ªú¿ú+ÀN°µˆãhñÀ;JÅø5À<«¤¸²@ Î
ŽÞՎ?ÿCýrr
?ÅGQù#¿'ŒÛñH?ÐõêÓH@Š‡À©(?퓿e=W?áÅÂíOú¿â¦ìq­Â¿ïÿêf:Ç|?ïÿž{€©ß¿á¨Ðº%*AGNbll3FGL J2307.4-12081RXS J230722.5-120520?ïþ¯X¦<ô?)ÕW\-E?%
tw¸m?)ÕW\-E?ïï%¥‰š|?cFP‰Zz?`ÚZDë$¥?cFP‰Zz?xºÚe?×ÍVÁu?ŽYáÀZò?×ÍVÁu?ïÿ'Æ&ü?Ñ)-•,?NfLكé?Ñ)-•,?ïøÑs-QÐ?SOe"iŽü?Lº2["ïÍ?SOe"iŽü?郎•¨Põ?‹<­ÛE
¡?†Ôڒ|&¿?‹<­ÛE
¡?ïm,Õ1[~?'œn*íùÊ?'ZeVdôH?'œn*íùÊ?ïý=Ã?@Ôñ|íã¼?7¦_x4?@Ôñ|íã¼AGN4FGL J2307.6+1451?är#ó>|ÀD…Å3À:!ó¥~ª*À<*¬3Ð%@AÎ\
m?ÿä̝Òä>?Ä;9ýQÏÖ?Ì
ɲ'@¬Á^ڀê@G¾Šß¿çëi~J‰¿ç¡ŸÒò¿Ù:€™îS/¿âßN_¤¿ä:aûš°¿é{bŸÝVAGNbll3FGL J2307.7+1449MG1 J230734+1449?ïúwð§ru?F4(šã¤Š?F =Çêš}?F4(šã¤Š?ïíP8ã²~?fª¡Ãx?b¯Æâ"©?fª¡Ãx?ïܛ	c߁?r§&ÝÕ׺?q²{/Ó¯£?r§&ÝÕ׺?ïýþ™´­­?wk?~%?00Kè…?wk?~%?ïû(Ô_"?D:¢›åü"?Có\Œø¶€?D:¢›åü"?ï¤3Xœú!?Žÿe_Ý¥?†ó)ØÁw¯?Žÿe_Ý¥?ï'"Ώ?Œ±`­]Ï?z8ìŠÌ/?Œ±`­]Ï?ïúMµ¯=µ?9nðz8—?FÉ)§¸?9nðz8—AGN4FGL J2308.9+1111?Çý›G׍ÀF)Q֌i/À:¥àªÐ"ÃÀ<uý'w>%@öª'».@(…ZGt3?ȎpÜ.1?Ò«3À ìà@3Äz@a¦ˆ›p¿ïÿúŒ—Ó?ïÿÄ}îB¿á¸rØd°"¿åVõ°å_¿ìnç©Çå¿°ûUvT4AGNbcuMG1 J230850+1112?ïïê ¿ ?a.HzŠ?`_&Bí5?a.HzŠ?ïãT[!
í?pUp{m¦?l«¤œù"´?pUp{m¦?î¿taѬ0?•"EPúÁ?¤¹ç0À?•"EPúÁ?ïÞéŠÑ2k?V
-öžZ†?p‹:Y†Â?V
-öžZ†?ïê €a?ePz*æK
?eß㪇Ç?ePz*æK
?ïY¢˜ÆµÜ? Z¿µ?"ˬޒ>~? Z¿µ?î-aª"é‡?Ÿ
Kâ›?­)åUՀ˜?Ÿ
Kâ›?ïSƆÙñ?ˆï3"CC?•œG2"]ã?ˆï3"CCAGN4FGL J2309.7-3632¿ïP¶)$ðÀP¡¸€®À:&AؤmÀ<rÐîš}@Í;­*E#@,™»þHp?´ '§7¿•ye»Vê?áìi ,°¸@¿­QÝBf?ïþÖj€˜¿ä\º:#è¿à5ŽÂ¦^¿Úr¼€Nnù¿â'—|ˆç›¿ÖàÀ48ñAGNbcu3FGL J2309.6-3633WISEA J230940.84-363248.7?ï8'Ñ?¿ºË,Ž©?˜ý/±—"å?¿ºË,Ž©?ïç¬#ßÙ?qi.hXd?hSÛÜΏR?qi.hXd?ï7‰lû¬?–ƒœVD?™Îׇô}?–ƒœVD?ïåþ‰TÊT?S½©>3^«?jvq|<7?S½©>3^«?ïߺE"<k?x""H&p?p"Ý,òÎ}?x""H&p?ïjøåë'ò?œçV#Œ?' ã?Ì?œçV#Œ?ï""ÆÓ¿?™Úæ¥lßÈ?›»§8þ5?™Úæ¥lßÈ?﷋(T³?mw¢|­×¿?'8ùZoC?mw¢|­×¿AGN4FGL J2311.0+0205¿æ"Æ`÷çƒÀJºÇË)À9n‹îNÀ<*ÀY!†@O²(؇@Üðû?±'®*?¸UW༘Í@HçÖyõ@'~k)¿å•XA_›Ç¿Ê1V?Qпâ*È˶LX¿çy]ä☿ߺ?<¿ë…Ð>qT×AGNbll3FGL J2311.0+0204NVSS J231101+020504?ïþÃ&Û¶õ?Ñû1]é?#͔ò©]?Ñû1]é?ïî8µÜ£ã?e£¹c$›Í?aÇJK7"Ì?e£¹c$›Í?ïßÍÒJ)?tÝUuó58?p¹?PG?tÝUuó58?ïÿwÔÓ?	>ÉiªRš?1c'E!?	>ÉiªRš?ïþJü "?)–g"D#[?+^Lx¿™?)–g"D#[?ïŸKüœ?Žz+"=T?ˆ-ã+"??Žz+"=T?ï«)`Ã܆?ˆ´)Xbƒ?…5§à6ê€?ˆ´)Xbƒ?ïþ©V{?"öçöÃg?/EnB"–?"öçöÃgAGN4FGL J2311.0+3425?ïǦ*TEÀ8煵·À7Òv pMpÀ;žq—òÐm@ò E>y@ëDå^³?˜lð÷¬ýØ?¸YaL1‡@nƒ
áÛ@l7ñ³áï¿´º`
±Ä^¿àÈÊ^³i¤¿å˜9²©5¿å&[^u6¿ë¡ê Ðâ¿èç=@Ó.çAGNFSRQ3FGL J2311.0+3425B2 2308+34?ïôëø[?U.u—{à?VyÖòFÚ1?U.u—{à?ï߂y@?wTtÇã9?p>Ã_'Ä?wTtÇã9?ïbÿˆÙ$k?'˜h›W±?" írx‡?'˜h›W±?ïþ1݃åd?"}Ö?,â*dÃj'?"}Ö?ïïb#"7c?`E•ûÈ?w?`ÜYê¥x?`E•ûÈ?w?ïlœÏÉë?¦s¾H¤¢?'lf >"?¦s¾H¤¢?Òs³_?¾%y"7?‰Ôiò`P?¾%y"7?ïù˨+úý?@-PžÒ?HÑ`äH?@-PžÒAGN4FGL J2311.7+2604¿äÿ¢¥0üwÀ? ˜€"åÖÀ:)Ö¢8¤ŒÀ<Sæ
ær@®¦xÓ{@!§ýàk?¼m<ïI¤d?©ÍáʵÆK?뙟}^P@•\Tê"?펄'¡WÔ¿áPž1Ú¿åà iA¿åé¯nî¿ä¯^'AcM¿ïë»MlšAGNbcuMG3 J231144+2604?ïþɆh±½?'}+oRÀ?#gœÿõ?'}+oRÀ?ïñ/.Z #?b%Ò7õÚ?]¡¢çÊù¿?b%Ò7õÚ?ïóÀ𱿑?c6‹±^?X~Ö:Lî?c6‹±^?ïþH¦¯Ã?TH?v¾?+ušÁvÕ7?TH?v¾?ïþÿ6×W•?ߎqmÿ9? û7– ?ߎqmÿ9?ïɎKݤ?ƒICòôUß?{8Úm
¯?ƒICòôUß?ïïNò¬Zf?fºÝ/?`±
d#¹k?fºÝ/?ïü¢"ü?/Õf®2??JëäÜj,?/Õf®2AGN4FGL J2311.8+4541?°¸Èx0;¨À+}´í²öbÀ:ˆþ{À<4å†×õö@»›¢|@|ôètÉ?Çï­7OË?ß"š‰®•?÷ï~Þ,p¡@×mŠNÎ?ؑÃâB׿âÈñ EØ¿êI
Z[–)¿á1‰Ÿü_7¿ïÿø]Ê5™?íÕx™]4AGNfsrqMG4 J231144+4543?ïœÏî☳?³qžöHØ?ˆÌUC?³qžöHØ?ïíF^«~k?d¢|ÞJ=?b¹¡^ }?d¢|ÞJ=?ﲸÍD›?'ƒ>ÞÁý ?ƒQÌ­ðw"?'ƒ>ÞÁý ?ïãUàå¼?TfïN4[?lªçi¸®?TfïN4[?ﲟ7úS?ˆ½SØÑ/6?ƒX1ÿ³RH?ˆ½SØÑ/6?ïkÛe
mH?™®"ik¼W?'""e1Ží?™®"ik¼W?îؽ'¤
i?™Žg!ÒV²?¢t&âO½n?™Žg!ÒV²?îÈö³s:?'¼|,'N™?£p"Õ^?'¼|,'N™AGN4FGL J2312.5+7241¿ê"T¢]|L@&xaՈÀ:Áñx}ÀÀ<4^[Õê@Uyqk'@{¹Fk?Ȗ³á‰9?פõ'Î{ù@¶l£—I]@¤Ge_M?ïÿï9_J¿ÙÃSÜöæ|¿â§§^~:™¿æ……t¿éþ	ù~¿ïüÓ$Õ¢^AGNbcuCRATES J2312+7241?ﯗ°
tM?²O³ÛœðÒ?"ò6Ä?²O³ÛœðÒ?ïåGC¥5?rãÊ`P¸?j¸¼¥²?rãÊ`P¸?ï<"Ȳæ?Žll¼v%g?˜ofþqF?Žll¼v%g?ïÒ£	8³?WÛf7«^±?v®{€bf¬?WÛf7«^±?ÿcè?‰¿%?~¹¢«d?‰¿%?ïRï±ß>?î¢Ù‹?•¢䜮>?î¢Ù‹?ìޅ4:wÔ?©WJ¬°ÿe?¹Ö\âfä?©WJ¬°ÿe?ï
0z1Ü?†8—dúÅG?ž¹ýë'Z—?†8—dúÅGAGN4FGL J2313.4-6922?æÍ¥d>:ÀF²SCsóÀ;Ÿ]ZN*/À<ë{o'V@"³u†iæù?÷Ϧ©?Δm_ÔÑÔ?ÍG,å;Xœ@>;¤ò@åÃèL°¿íu/¢/k¿ÖB²A±%Q?ïü÷"
í?ҁüœÌ¿ååwÞ³Õ?ÓPúïIúAGNbcu3FGL J2312.9-6923SUMSS J231347-692332?ïÿ)]t?ǽó<À?ÝDˆ?ǽó<À?ïö¶øâ?U4)DHaŸ?S'‹®*'?U4)DHaŸ?ïêˁ"?^5XΌŽC?eý5:\f?^5XΌŽC?ïüMÀŸI?3F=ÏÑJå?='úÿÎð?3F=ÏÑJå?ïÿ‰)¬C7?G7EÛ«?
µÉ›íQ?G7EÛ«?ï՘Ÿ÷í?ƒÒ)ò»Ë?u3°gVf?ƒÒ)ò»Ë?ïëcnöi?nGpoQT?dœ'<q)?nGpoQT?ïødKʗ?HéÄÜhÎ,?NnÒÂZËq?HéÄÜhÎ,AGN4FGL J2313.5+3945¿ìÆ[žâ-ÝÀ3U<¼M#À9³¨eå7'À<!ܘòª­@½sßrl@=ŠT'8T?»òÂ?U*?ęÎØþ´@¨«ÕÜ@@`äƓ¢µ¿ÃÔ¤¯ò¿æl{=ãæD¿é¬MÑD*Ò¿í(~#qt¿àf6`]'¿ðAGNbcu3FGL J2313.1+393587GB 231102.6+393314?ïý.Љ+?3j§Ä‰QÊ?6‰|Úñb?3j§Ä‰QÊ?ïò!Ώx6?c[ö]Q?[¼c‰óq?c[ö]Q?ï¿Õh°K??z¼x(6Q?€
¥Ø¼¤?z¼x(6Q?ïþÏÄ#?Xˆ'.	?#»eÁä?Xˆ'.	?ïýEÂú2ƒ?8¯L[Ù%?5ÑçŽþÒ?8¯L[Ù%?ï—ƒƒœq?†mt4 ¿ª?~´>>1ǁ?†mt4 ¿ª?ïE÷2?"ùò´bÕ?ž—_ݪ"z?"ùò´bÕ?ïúˆ~-[?8[—xHކ?EÞ?Ip?8[—xHކAGN4FGL J2313.9-4501¿¼Ï£ä¹ÀOÊìë¯À:R€;$À<FÅA¾q@½UzþÂ@H.D¶é6?¼/©Ýˆ\?"Ö^úiñ"?ÐD4¢Éî÷@dÕcIP¿æ"G!ý¿ã?¾&@Üi¿êù­ ·›¿ëÞµbLü2¿¾"V7$¿ðAGNbcuPKS 2311-452?ïÝR2À ?­ð¢÷³¢§?qVæÔÓ[þ?­ð¢÷³¢§?ïõ{e¸&ß?\ðû£J'?U	44"Ò?\ðû£J'?ïsQxî~M?ÆeÌ§?'•ÐåŸÒO?ÆeÌ§?ïÿ‰tÕ·O?›‰Ê/|?
¢ºZjÜ;?›‰Ê/|?ïõãœût?bæÕïÛ¤'?T8ÅÚBhÊ?bæÕïÛ¤'?ïØâòÓò†?uЎ'úÌ?sŽ†©ôxí?uЎ'úÌ?ï+N¶?kõ$7uk?œ˜ÛÃ?kõ$7uk?ïû•p¦B?@bzÅ(?CѪÊ#Åú?@bzÅ(AGN4FGL J2314.0+1445¿êçoD¨ÈÙÀDôsš¿À9¶L¨O?À< >ÏH¨@ ajNÚY?ü¾ú1‰æ?µίP7?¯Ø\"Ó?û½CÂÍoŠ@JÆ!âÔ¿Ø°îŸÛR!?â盺Ü	¿ÞßÑ ïcÑ¿ÙT)McÓ¿ÞþGï¿Ö›;$™<}AGNbll3FGL J2314.0+1443RGB J2313+147?ïýN'ˆãœ?'`mn÷?5ŽÂt‡ýí?'`mn÷?ïè(ø‹†?in?÷ ?gú×"ñY?in?÷ ?ïñumaÏ ?afRcø.?]$ì©Ð?afRcø.?ïØÂ,‹&?W‰Môc{?sžê—%
?W‰Môc{?ï÷ØdÍ?G¯¨Í1?PO×¢³B?G¯¨Í1?ï•Ñs=?•:TÞ«Q?Š‹œ˜áê"?•:TÞ«Q?ïêi1ê*M?rÞUúñ>?e–ÍòÃ
?rÞUúñ>?ïvä˜üy?}Ø ŸÛ·?'#lýÀpÚ?}Ø ŸÛ·AGN4FGL J2315.6-5018¿»viO
:}ÀN?Žâ†ruÀ:3"_ôöÀ<zäÎKR@×5›J@N_œGÉÃ?»ÐßoÖk¿B'Â%™?К©#¥K©@=tю'¡¿ëåN¾©ô[¿Òe­ÄHﳿæê~Ž{X¿àµâoÌ@¶¿îÌaË¡ÿ?ÏÁ¡
&I–AGNbll3FGL J2315.7-5018PKS 2312-505?ïý›ˆuô"?'¤BÒÕÓ?3#¾séô'?'¤BÒÕÓ?ï÷F"ÀÅ5?T9)ò`½×?Qrض=?T9)ò`½×?ïË·_ßö?{[zðL0î?z$wRϵ$?{[zðL0î?ïÿ}˜Ôo%?ø¿ÎTBì?Lß©¹xú?ø¿ÎTBì?ïü£R'-¡?6spûÏ?:åkª@N©?6spûÏ?ïÙëÆâýç?€ÞHsÙåé?s
!4²?€ÞHsÙåé?ïÐKÝN$P?€ìf"…u?wÚX=ëà?€ìf"…u?ïþ`'Tz"?#ô\ݶý?)ýŠ)nP?#ô\ݶýAGN4FGL J2316.9-5210?Ój`ДoÀM­ÝiÓÀ;)û¤P¬ÁÀ<ÐÄe¨Ñ@ T
$Ç	¿?û¡Îl	=–?ÒÑE= ó?¾ùÝ?û\q?çt/è%ç?ÿ©F«
/Y¿æ5à¿ék×3X¿ã¾+Ÿ@!®¿Æßjßÿã@ä̝Òä¿Ú½†þâHµAGNbll3FGL J2316.8-5209SUMSS J231701-521003?ïþé·ê¬?!41ÁÚ?!d…~m7ù?!41ÁÚ?ïõ{ç¤`ê?W÷ŽùùÇÕ?U12êç?W÷ŽùùÇÕ?ïòd
ƒ ?VÒ°î 3H?[7䡖on?VÒ°î 3H?ïü‹\G²$?$é?äç^À?;¥G?$é?äç^À?ïþáÔ¾*??=bÔ*þˆ?!â±õgžÈ?=bÔ*þˆ?ïÒÀÚ~?'As˜ùª?vûŸå5hà?'As˜ùª?ïó?÷«Œz?cèžÝw?Y€Äcëº?cèžÝw?ïñuÝ
?QÆ^#ñԞ?]F/ý…:?QÆ^#ñԞAGN4FGL J2317.0+3756¿ëoߣíÀ5GvĂ{pÀ:ĚŸ˜·À<K¯)M×#@Ñ·gµÇ@AËÚ^…Ç?Ë´ge¿Í`?¶­¾,0
?æqËtÝø@ížÏ
™Ç¿çæüÞãOƿ⸝Ö?<V¿áF%žu "¿æ°Ì@Šß—¿ïü•aütZ¿ï¾áÝU03AGNbcuB3 2314+377?ïû­âj²•?8?ŠÆ/ôÔ?AHv1y»~?8?ŠÆ/ôÔ?ïðÛ´­W?`SO/j±?_ÊHI®{?`SO/j±?駱Y"ù?'Ù÷//?†Ù~f+eÜ?'Ù÷//?ïë2®S?L#®[lãP?dÍQ¤±Ôe?L#®[lãP?ïú¿é˜?A ÌnN+x?Dôÿ"tÌm?A ÌnN+x?ïÂÇ~•mv?ˆ tîÙ*î?~œ@ÖE"·?ˆ tîÙ*î?ïy¤Mʾ?Ós+	?ËvKæÒ??Ós+	?ï‹äµKÑ»?zn.iô].?ҟM!l?zn.iô].AGN4FGL J2317.4-4533¿îD´° nµÀOâI@¼À:/e‰Ç"À<Vè³³ @½EªI6?ü¯§r 0?º2€…Ì];?ÆǍȪÿ@'3@˜™is?ïþ.~Ãq¿à2÷~|1Õ¿ØTü܊%¿ÝTVc¹ã¼¿ã~¬ãù9<¿é^­'*AGNbll3FGL J2317.3-4534SUMSS J231731-453400?ïû1AÊv?ClOåÜÕ?C:ø¾™¬?ClOåÜÕ?ïó'íkäç?bû?&µ,?Xú$ù{'à?bû?&µ,?ïÎÓQ°;?ygcs8M!?x–vav¶—?ygcs8M!?ïøjû .?5Û¡¤ƒ?NTRÙkX?5Û¡¤ƒ?ïúmâ[ªK?D«"ŠÐ¥?FHué©åâ?D«"ŠÐ¥?ï×j™•¬"?xJeùáÝE?tJ³N;?xJeùáÝE?ï`éR5?4BÛOz?"âÕ¼y\Q?4BÛOz?ïçpiÄ?W0Ó05÷7?h菐t3†?W0Ó05÷7AGN4FGL J2318.2+1915?ï9z$‰LDÀC4t}€^_À9²Áo¡x‹À<Íê>y@ËO¤@I´˜c9?¶Ì—Þ-G?|¿ûûZ÷?Å'T,þ@,½£9+¿à\VbbJοæ–{(,¿é0¸.°¿àÆးø¿îE·Ï冿ïü;ºÁ1ŽAGNbcu3FGL J2318.6+1912TXS 2315+189?ïü‰ga&û?.ÚpÍ+?;´ÆŽ³]á?.ÚpÍ+?ïñxA…4?b æ¶ùü?]}•¼É)?b æ¶ùü?ïå2
C_?h7v¤ *?jôÎZHh?h7v¤ *?ïþLó½kJ?PX¶/{?+0ÁŠ—§¶?PX¶/{?ïý6o†SI?7E،[eÝ?6Lå6Ña?7E،[eÝ?ïÇâŸ>k˜?¾è1Nûê?|°JÈ$?¾è1Nûê?ïá\ÙÊ·?t›É6ϦÅ?n£&b£¹Ý?t›É6ϦÅ?ïû†Õä?:|UiZh´?CáçsØ~?:|UiZh´AGN4FGL J2319.1-4207¿îǪÜë†ÀP|+IºÀ:uú=H_ëÀ<•æÉÎ@,ùÏdVÂ@.Øà×EÍ?¹oÛÛ£
¿ŠŽÈvÉ?Ñ«Dœ'x?ý6"y þ'?è÷Z_G
[¿ãmü\ÝP©¿à'Æ-Vпà…à19¿âW°ö­pç¿Ûâ H£ÞAGNbll3FGL J2319.2-4207PKS 2316-423?ïûi3[ˆM??=~S£Ôq?B[2ò —ª??=~S£Ôq?ïóا¡o?Z?UÀi¸?YøNBÉ¢M?Z?UÀi¸?ïî6¾ÐW=?f‹S'뼇?aÉA ŠzÊ?f‹S'뼇?ïó"?*Ò?DûVh8™?X×Ï,tw?DûVh8™?ïø'2IÔ4?G»Aõãr?M÷6ÿ·ŠÂ?G»Aõãr?ïÊ,SÅ?'ç5ª~"?zé±sMÕ?'ç5ª~"?ïí–"aû?ohºëÚ?bi䂛…=?ohºëÚ?ïÒª•HØ?dÿB6A??vªµ\­ÿÒ?dÿB6A?AGN4FGL J2319.6-0456?Ú4ssúÀMkøüÖÔÀ:ü8ç¨fÀ<‰á<ÆYì@ '¦un?ú ˜ u?лR;Œ/?΅xdë'
?ÿ•S¹»@þ€G7w¿ï嵜.ŸP?ëýQÏÖl‰?•	i¤ù
¿Ð:n%wˆÎ¿áj3°0´Ô¿áI€|'!ÖAGNbcuNVSS J231929-045640?ïüµ®UÆå?0E®§%8?:RŒª¨©l?0E®§%8?ïåó<«µ"?nÉbw(ƒ?jÃ-Îܨ?nÉbw(ƒ?ïÚ~ªïœ?sýª½n?rÀª~"Ô?sýª½n?ïäAÖd%D?RŽFg‹!?k¾)Œ¼t?RŽFg‹!?ï÷elåä?L",Qªˆ"?Q5'_ƒˆâ?L",Qªˆ"?ï~lƒ¥«:?—®kEšÕ3?2o')ÐÃ?—®kEšÕ3?ï̳ûÝ9?}ZãÑSÃ?y¦rýAïm?}ZãÑSÃ?ï¦x¢~¶?x­=µuÑ?†a×]	öm?x­=µuÑAGN4FGL J2319.7+1609?سá[-ÀDªiƒQX¸À;/=÷²S¥À<¡ßòC~Û@ ¯´õj¥»?ùgk´"«?Òãk¿ì""?Ԕ–e¿ã@Á}ä1@düsÙk—¿ïþ›vóQ?ïòh!ýU׿垴‹g\¿¯>'iÈ¿á×U¼Ê÷
¿ïó¬ÐDÑAGNbllRX J2319.6+1611?ïûR-?6¯¦6ÞK6?B·ô&µI?6¯¦6ÞK6?ïÒs¤VOÝ?'uA™·?vÆ-ØG­¨?'uA™·?ïÆ]àŽ~;?sí§òz–×?|Ñ¿ e?sí§òz–×?ï˧*HJi?b£Rý[ó?z,jè9cq?b£Rý[ó?ïû\Ý{›­?=±Ha'?BŒŠ®?|?=±Ha'?ï*Ӂƒš?¦Š˜?š¥ÓˆÄ?¦Š˜?ïÅú+sD?}F²}&'‡?}ê}¦5Â?}F²}&'‡?ï7)¦±I?'Ú»h~?ž9Ælè?'Ú»h~AGN4FGL J2320.8-0823?æë7';ÒÀNőÙýÀ:Ÿ>ÔI™À<Q˜hA1ù@j×9bL@2Á¾{Ñ2?Û÷Ü°ožô?Ú+ഐ@@¹áåéÔ@	P§d?ïûU@¤4þ¿ä©ÅÌ'‹_¿é€¾×@Ä¿ë‡Làƒbö¿ïõN`¶#=¿ïÿ%D]'#AGNfsrqPKS 2318-087?ïöUFOçì?RåøiÌ?SUs¯ç3?RåøiÌ?ïáO6…3l?wÌ(3ˆ?n°Éƒ£¥?wÌ(3ˆ?ïf,š<×¢?…k«¹p"U?":l»Ô§Ä?…k«¹p"U?ïÄfeû"?c÷È|o¸?}ÌÍe³iù?c÷È|o¸?ïíúozêµ?k͋™:Ì?b•"ju?k͋™:Ì?ïf,GÍõ?Ÿô4$1Ô?":w&%yN?Ÿô4$1Ô?ïs/ç?'pœ&:?œ±–¯g3?'pœ&:?îÇë5ºïL?&	°×˜?£L¦äÀ:?&	°×˜AGN4FGL J2321.0-6308?»i—¸ÛÖÀIŠiƒQX¸À;[ìëPFÀ<îUsÏÛu@ ;òÈ	­?ýDÌh"ÿ	?ÉX°›>?À¤ÿ§j"?ó홖>›F@nr
—~?è¿Wߣ¿éì¶wò?³
|%js¿áMÚ~f7l¿â>™˜ÂÚ¿âw®aÐ*AGNbll2MASS J23203986-6309181?ïþMîþÙm?"=`ÁKÖ±?+!ÎÈ5?"=`ÁKÖ±?ïôYlåö?Wúÿ	gâ,?WMö­AÔM?Wúÿ	gâ,?ïò­ç¯Q<?`¤™Õ7*=?Z¤0m#x?`¤™Õ7*=?ïô}ù*"é?>ÛÑìwR?W$¬læ?>ÛÑìwR?ïûñ®a/x?::ÒÃL?@9G^Ûp2?::ÒÃL?ïÕÔÝ+X?€>Z\+ŸÍ?u'z!íX?€>Z\+ŸÍ?ïóËW'õ!?bz'îÄ?XiPibŽÒ?bz'îÄ?ïÛQSž|q?a³ra€ò?rWV%_•?a³ra€òAGN4FGL J2321.4+5111¿ÞêÅ
ï5À"hæŽ>ò"À:7{~% À<H¯¤Ùš@þI'¼1Ÿ@SüC²Ý7?¹2·ÖEœ?ha[¿¸J?±ww°»Ÿ(@dš´KÍ?âmy_èGý¿®e!0Á¿éõP¯Dü‰¿ÕXÅÉ£M¿Ñ¿

Áû¿í)\_§ZwAGNbcu3FGL J2321.3+5113NVSS J232127+511117?ïý%˜ü÷É?HΝû‹½?6Ó7µLø1?HΝû‹½?ïóòʧ~?]@kO6MŠ?XjÍCä2?]@kO6MŠ?ïóÚזC=?IÇTÜJdˆ?XJPhE·6?IÇTÜJdˆ?ïûiàÞ?+Ûöè×}Ö?CîXyÇùË?+Ûöè×}Ö?ïôÎJȝ‹?YþÁ¯ÁÝÞ?Vcj˜:®?YþÁ¯ÁÝÞ?﯐h°™?"Â3¯?"ÿ÷åÄ?"Â3¯?ïêøM?rûÿ=òY?e~ðÆ3?rûÿ=òY?ïðW³g˜b?NXC!D?_P™FÌ»Û?NXC!DAGN4FGL J2321.5-1619?æ?¶ŠÑDÀP¢øa¦
EÀ:2íÈÅ×À<PšíV°@ R""Fô[?û\ãJ½"t?¿']è¾oè?¸½ßÉÿ'ó?ü`q$/Š1@Òú›½
b?ïÆ•Q5}¿æŸCâ­ß¢¿ÙoD]¿ÇM»à~í¿ç€N9Hö꿧Û7TAGNbll3FGL J2321.6-1619NVSS J232137-161935?ïþή	¤U?ð˜´1Ò?#"ÔVr?ð˜´1Ò?ïîñ9 ‹?dv<ÄÖR?aû軍,?dv<ÄÖR?ïôG%-Œ?Qõ'<ïn?WÝq73H±?Qõ'<ïn?ïúÅ«?1ϙ!gZÓ?G"ìn¹Û?1ϙ!gZÓ?ïý•ˆy?/-8ߋÍ?3S¼äØÕ?/-8ߋÍ?ï«ÔB"?‹³ ·ã4,?…
øƒ>K[?‹³ ·ã4,?ïäœËÿ!?tOshÊ?kc4àã×??tOshÊ?ïô7‡«°r?F€A~ŽNâ?Wð¾œšï?F€A~ŽNâAGN4FGL J2321.7-6438¿î€~®0ÕÀHì° Ä›¦À9µKÀ<p¨O?t@Šû"@ÈqGÐ?­;Ì´Îÿ,?G•๗%?'Õb垼@»¨pL\¿àp¦€Ýµþ¿ÞŒ'àl絿â>=Áç¿á»i˜JA¿å(ǟfb¿» ×»é$ÇAGNbll3FGL J2321.2-6439PMN J2321-6438?ïÿ`›K?
YŒ¹û?sø"VÔè?
YŒ¹û?ï÷ØýeN—?TͪÀÏè²?PNô=m¯?TͪÀÏè²?ïöø[>«?Nצí9ð?RIíŠß?Nצí9ð?ïÿöîô>Î J[
P>Òäq1ž>Î J[
P?ïÿé˜4•?ܤ¦²Íu?'Ñ窯¯?ܤ¦²Íu?ïâÿé|'e?nèŸèÈhÕ?mƒØš¿?nèŸèÈhÕ?ïõÑtÁè?dËiq·?T]Ù.ê?dËiq·?ïÿöÌ5ßF>Ðgˆì¹»>ÒgR=±©1>Ðgˆì¹»AGN4FGL J2321.9+3204?ÙÜ€xá=À;ö<1ßvÀ87[‹ABÀ;‡³äžzª@Øם
gb@Hƒ&Ž? 'FJƒ?¿ò.±fS@ý"$½@Y0Eíõç¿£G>ÞF·¿Ýû†ß؝¿ãJ|àü.º¿ã¬fZ§ìC¿é袠ÿ>¿ëB&¶M.‡AGNfsrq3FGL J2321.9+3204B2 2319+31?ïôGq)?Ujǀ$$?Wqèï"þ)?Ujǀ$$?ïáÃ;Íû?vqœy.å?n<|ÂÒ,È?vqœy.å?ï©<QP;?ˆ/~'¹"?…¿°è<UK?ˆ/~'¹"?ïúåLSg?9'É'«?DjϾ¸Ï?9'É'«?粒Ö-§6?ˆ9ö\.?†Šch&§?ˆ9ö\.?ïKDOBæã?®¶V[ßØK?–—v{¹§?®¶V[ßØK?îØÝp‹%?™0oªÚ?¢sÆ)Ó4±?™0oªÚ?ïèÂξ‹ä?^˹7Ž?g=1›$?^˹7ŽAGN4FGL J2321.9+2734?å5Ë	À?;Y5ü;OÀ9"¸ÜU
À<4›ök+È@w>ÿ¥@¦pâÁ*Ø?³¤ëÝ3L^?¶Y"€a'@³â…›µÔ@ܰљ4?ïåѶ@™M¿Þ¡NÄ´$Š¿äœ<I	^¿ÜmÍ"ˆ8¿è˜¢ô¿åt¦FPFAGNfsrq3FGL J2321.9+27324C +27.50?ïû؋qã?1þ(9yL?@Ó"úD?1þ(9yL?ïÛMyc ê?'Xÿƒü?rYC5o?'Xÿƒü?ïëAPW[?m5ËXuD?d쾃­¤á?m5ËXuD?ïQûtY?{Â(@R`ä?•Ð–¥^Ï?{Â(@R`ä?ïñ9Ëu+H?WÑ@µT?]Œi†\ ?WÑ@µT?ïd¾NÀé{?™	q«¯iç?"h6"»fª?™	q«¯iç??ŸA?â{âC~?ŽWpÀx?â{âC~?í.<Dî‹R?ŸpÞ¸¨?´?¶ŽÖeãñ?ŸpÞ¸¨?´AGN4FGL J2322.1+4440?Œ}ìÀ.·¤ƒ§ À:©È"h¯íÀ<\§D}"@Çs){r@'ä´J?Ë}õ#XÐ?ÉÓQáŸÜ@]týØÞS@þ#ØÍ6)?ín«äõ¸~¿ÙpfÅ[ê7¿æåà/Ò¿ßnwa¶Sd¿ìðZÛî¨À¿ïõ_¯"AGNfsrq3FGL J2321.6+4438B3 2319+444?ïÎy÷ª?s‡°£¢b:?xÃv‡§ÆÜ?s‡°£¢b:?ïǚf{½™?ìO^	
?|2ÌÄàãd?ìO^	
?ï…m&'?¾äƒÚ	?Ž¤¼‰ôæ?¾äƒÚ	?ïA•µoŸ0?r¯ß0p˜ì?—ÍILä¯ù?r¯ß0p˜ì?ïaMI¬=Ø?‹Õ0»¸$?"ÖVÍçàí?‹Õ0»¸$?î¯Û/;+û?¦Yí×o)?¥MqYQ?¦Yí×o)?íبV\b?Ÿ}]t©<?±:½LC}î?Ÿ}]t©<?ëÂ<ub"?¡!—ˆñv?À÷'*u±?¡!—ˆñvAGN4FGL J2322.6-0735¿ëThÌaîÀN¤gbèÑÀ:|©B"	À<Vhiuå_@+ëÞ
ò@bå€!ùO?Ä­Îq?²½)썇h?ìrAÁ@|@|e´å¥a?ïÿT>Eµí¿Ö7@¿åº#ý¶#¾¿äc4^ÁV¿æ6_½Õ¹¿ïÿÀ_V&ÓAGNbcuPMN J2322-0736?ïþ}ì¿ÜN?Ê2zδ?(!0
H7Ì?Ê2zδ?ïîÂà‡67?dìÚ´™¿?a=hK©?dìÚ´™¿?ï쌾g¸?bN
Wz?csAnößñ?bN
Wz?ïþ]¯øD?óⲡ)?*%‡t"T?óⲡ)?ïþ‰›Ô×?#ØØ¡¶?'fMh%?#ØØ¡¶?ï³¾1î(?‡'Zš§Ìè?ƒsyÏÔ?‡'Zš§Ìè?ïÞ¨¢©–E?tK« hùé?p«®¹£9ª?tK« hùé?ïüP'›È•?0r3•­øˆ?={ê/ÖÖÀ?0r3•­øˆAGN4FGL J2322.7+3436¿çoAL·¤ÙÀ8Ê!§´ÝÀ:ñ
™¶öÀ<T_°i¿·@ 1͒ð] @'5>¦?²Ûù ÜÚ¿¨›ˆ²¼U?öôÖ¡aä÷@BY@ãö¿èŸÁ¦Óê¿ÝçK~-­b¿å§Éþ;YÈ¿Ýu=äçöŸ¿ØºËã˜Á-¿ÔÔúc
AGNbll3FGL J2322.5+3436TXS 2320+343?ïýõ5™w?!ø÷q´@?0VQGÃþ?!ø÷q´@?ïð¶oµ'?a6ºWyl?_ô'Ùü?a6ºWyl?ï÷Ñøzƒ?D©6ÛFe?P]ł?D©6ÛFe?ïõ`ôR?:Dâs;îI?U?áôԌ5?:Dâs;îI?ïüOÜ-µ<?2Ötç}J¾?=¿:ë$?2Ötç}J¾?ïºÈßq.?‰Þ•X¥?|MÅƒ?‰Þ•X¥?ïô15hS?iPº;}j?Wϝc´úƒ?iPº;}j?ïÁíd5Î?jâ€×˜*?~	C–Dà?jâ€×˜*AGN4FGL J2322.8-4916¿™Ë˜š@3ÀO´á¼©À9ʾšÚâ9À<
¦{)l
@‹]"•{}?ùÉ¥¶Žj?¹­®#"Y¿?Æj Û'G@ܸŮËZ@ã¸>Jh"¿ïý2%9þ?ïÿ"D¾Â¿Ô¹`¿'F¿Ñbf¼ønf¿åǞ?È¿×pŸ$rüAGNbll3FGL J2322.9-4917SUMSS J232254-491629?ïú|¨§I?Cm<€Yó?F
`mgø?Cm<€Yó?ïðz?GyÍ?w!|{Q?_!Uuµ?w!|{Q?ï¸Nµ¼?}óÁš÷ã?ìxLa"Z?}óÁš÷ã?ïô/y:â?Bø¶ÒTYŽ?W¡(Dì;?Bø¶ÒTYŽ?ïð»'ø†?`	Ò¡]?_މ÷†Ò÷?`	Ò¡]?ïÍ~U›gû?'—$Ÿqø?y@Õ!ö¥?'—$Ÿqø?îë=¾Q‰à?™|ƒGîb?¡L$S¬ý?™|ƒGîb?ïԀ¬Ê?k	òvòQ?u¿©æ¨G?k	òvòQAGN4FGL J2323.5-0317¿æjFDTe)ÀMO½­uÀ7勾åƒ}À;~^ÛWª@¿ÈVÆ`L@HAíá?šo7àü®?¸''	"83@¡e}'%@Éï"µ¿ÑTù²W¿Þ¸ô¾-w²¿ä¡:B-ƒ¿äxfÿš6¿éÏ¡þÂé¿çÞ7u¦AGNfsrq3FGL J2323.5-0315PKS 2320-035?ïöë ¼<v?K©ÇäÀ!?R(¿¸d!?K©ÇäÀ!?ïÝHóh?€ê›âöº?q[†"ÛÚ?€ê›âöº?ïћ¡9ø?|ŒŽ?w2/M°—ú?|ŒŽ?ïü>2g"?1	½Œåø?>mš‹ŽP?1	½Œåø?ïæ'a²?cÙ·Ð'ª?i}üÄ9?cÙ·Ð'ª?ïc¶©}oö?¨q5"Ù?"‰*Ò	ÏA?¨q5"Ù?ïª_½³\í?ˆ°bÃJ–G?…hú¸æ?ˆ°bÃJ–G?ïïßצ?ScyPlã?` )%sC"?ScyPlãAGN4FGL J2323.6-0617?¸ÚÚÈâ'?ÀNBàP7PÀ9õ¸Ú§€ãÀ<àŽµ:@‡|"P.—@é=¿Íá?»ðN²º¢?ÇR¿€#@	ÞRù¢í@׵̀?íri^¾Q_¿ÚˆüvÄ¿ä˜Pž¨ø¿èˆ4ýbÁÁ¿ét÷Ãñ[ø¿ïy
]QïAGNfsrqTXS 2321-065?ïïp»©äÀ?[—–¿´ˆK?`DK±?[—–¿´ˆK?ïíò.䢊?ey8¿{ãÌ?b
Ñ?.	?ey8¿{ãÌ?ï³`ë…Ó?zàBG½¡¾?ƒ'Å"[?zàBG½¡¾?ïþ†O(Ëë?Á­ýŽh?'›<ò¹?Á­ýŽh?ïÇNNôÒ?{¹e"äî?|Xø=¸£?{¹e"äî?突¡M©<?‡"/S?…š—¢FÜö?‡"/S?íšïOX­Á?¥ÑøÍâ?³(……¨…w?¥ÑøÍâ?ïü›à¬ä¶?-Å;ßì?; üU2`?-Å;ßìAGN4FGL J2323.8+4210?瀁ÅùÊÀ1ÍýÞ½À8«€U¾À;"wï$æi@L{)#Ù?ütwéR?¥ÌÁ¶2?±v¡G
Ë@.xžwNì@
Nv/²¿Ù#¸ÁÒó­¿Ò¢Ÿý‹Üm¿àJg,_œ¿Ö(ÑE'пÜzptb¿âÓ¿°.±AGNbll3FGL J2323.9+42111ES 2321+419?ïþ÷?3"?"ïº䶌?.pŠ…Y¨ý?"ïº䶌?ïé¿`Êèi?q
"ô	˜Ø?f@Ÿ7×G{?q
"ô	˜Ø?ïìž:%s?_IbÃC_?ca€Ç:dž?_IbÃC_?ïêÓï"'?Fñƒ@Èsé?e,óKöP?Fñƒ@Èsé?ïü(0ª?7ºÖ
ò'??~½Ë8Çß?7ºÖ
ò'?ï¦}°Yúr?'êz œFŒ?†`"écm?'êz œFŒ?ïñ6~õ±ü?p ‰ÇÆPý?]"ë`¸\?p ‰ÇÆPý?ï±lÃ(?mS7ØÜí?ƒ¤Ï4˜'?mS7ØÜíAGN4FGL J2324.7-4041¿¸:Cq|–•ÀPå6&,ºÀ9+þ¤¶-NÀ;¼çºŽÜ§@Øc1R³V?ùùÆ_ËA²?³1`n™€?µ©¸J´¯@å:a$Þ@H€ú?ÁʹÍÇè¿Óf$a´%¿Ý±äíU¿ÓryšÑW¿ÙÊûçA˜¿ÖìsԐAGNbll3FGL J2324.7-40401ES 2322-409?ïÿìʇè?	/ i–?b®DW?	/ i–?ïõKïíŽ?_, Ïî<?Týh€Yó
?_, Ïî<?ïð|mŒg?R}|éóÁ´?_%\´¢'?R}|éóÁ´?ïþŠ&+…6?>MnظŒ?']TÞM§?>MnظŒ?ïþ¸yH?åŒ/hÞ·?$xk"áØ4?åŒ/hÞ·?ï×A»"ɯ?€ü8¢—E?t_"D	"?€ü8¢—E?ïèKÿîôP?qÅ«ŠÐ°Š?g´8ç'™?qÅ«ŠÐ°Š?ïüÂl\Û´?0>®ŠwK?9ìœéÚð¹?0>®ŠwKAGN4FGL J2324.7+0801?ßµá聣ÀH†`˜À9'‹©ìÍôÀ<$_iòâá@[(+îz@"­ÿ'+¿?´¾¿iŒá?§k,Á "–?ñY×\rǞ@	Yh&/¿äƍm;¿Þ4ÓpsÛ¿äßd¥Ï2¿Ýx`«¿æ¤"…|+¿æòø°€eìAGNbll3FGL J2324.7+0801PMN J2324+0801?ïþ†_C÷?$vÁV&5?'š¶n?$vÁV&5?ïîlç°?f/E%ðÁ?aï"ߺ÷ø?f/E%ðÁ?ï÷¦ƒs"É?[þW?P²ùP´.Ž?[þW?ïõ6ƒØÞ?B_S"ԊP?U'ùàŠÓ†?B_S"ԊP?ïýJ·c?0e:­«?5ªEm°M3?0e:­«?陼Sõ(>?ÞÀÈ»#?…k
Äb?ÞÀÈ»#?ïöí£˜1K?^O+͓e0?R$¸"$J?^O+͓e0?ïÜÅ|1ºô?cB"ió—ô?qAý À?cB"ió—ôAGN4FGL J2325.2-2010¿ê&z²<—zÀQF¿]xÀ:ú"=_ À<¬˜ÜÛ7Ê@ Q$"‰åG@Ûþ +ïr?¾ôöŒŽÄ)¿´C?šÊœ?ó$5æ€Ó@"†ÔE,?î:ߎñ¿åM¤c!7ˆ¿çti>2пÕMW—Õt¿Ö(`¼ƒS‡¿áæ7¢-¼ÒAGNbcuNVSS J232520-201213?ïýÁ·Îk'?&iæWÒ÷~?1òB*÷ݱ?&iæWÒ÷~?ïì¦úUF.?ui¤Fa\h?cY±™
k?ui¤Fa\h?ïöA…?V¥r²Ö&?Sñ}eA\q?V¥r²Ö&?ïûªi[Êg?*¿|­÷Öþ?AV[J§¨?*¿|­÷Öþ?ïü€äÕ$?4ݛÀø:×?;ÿ*ÄÒ33?4ݛÀø:×?"¼$?Žé'¸üKÆ?‡'}Ô1¿?Žé'¸üKÆ?ï÷cò¡PP?Z©ø§"!Æ?Q8–ïë?Z©ø§"!Æ?ïè‡CçNj?[ä´¥N?gx¼
9´å?[ä´¥NAGN4FGL J2325.2+3957?Ðj'7ÛÂÀ3ûªy»­ÁÀ9	Ô¿	•«À;ßʯ¼Î@^(ÿI!?ÿãiÇCöÐ?¨É&O"?½–­@Zöƒ{á@GS&m§ù?ï)KRä©¿½§A"	?D¿âáÝ Y§;¿à—[µ2|¿ä\ËG'	¿ì
³!9AGNbll3FGL J2325.2+3957B3 2322+396?ïGöîM>ç?ÁæQ¸ÚQ›?—"9Ç¿?ÁæQ¸ÚQ›?ïÜ|p®?"®6ð¾)Ø?qÁ·ù¶¤¿?"®6ð¾)Ø?ï¶qøڋ–?"¿V r?'c¿FŠ?"¿V r?ïњ¶òg]?^x>µ²Pã?w2¤=-K?^x>µ²Pã?ïùdÙ¯šs?P.ç™ã³?Jl™Ÿ˜Oä?P.ç™ã³?ï6zTÒ6»?­Áê¯V‡[?™0µe¹('?­Áê¯V‡[?ï¤TitôÛ?ŒS»*@¤?†êå˜sõ]?ŒS»*@¤?ï<™MeÛÉ?'M—–iÎM?˜lÖ[یÈ?'M—–iÎMAGN4FGL J2325.4-4800¿ïVpšFèÀOž¡ß¹8›À9)ÎPZ‹À< }ðƧ@"E³"@ƒV–åŠ3?­RŒâŽS?£T<ò½?õc£Âˆ@2ÃÈí¿Üƒ€Þ6׃¿ánðx£Ì¿âÿ¾øMڿߜè"éŽú¿âár@<I¿ãY¯åC;AGNbll3FGL J2325.4-4758PKS 2322-482?ïþ¹²¤é•?~Uï9Î?$dÑØ=b?~Uï9Î?ï÷v=ÁN?ShÑܞT~?Q"%mê–?ShÑܞT~?ïõú¸~?c½Ôiªº½?TÄ
kFՑ?c½Ôiªº½?ïþ¼ÇàÄ?BG»ØX—?'ä1 Ò£¯?BG»ØX—?ïþ'¥:?YxÁ|È?'Þõ¬XÓ?YxÁ|È?ïßN	"h‹?rPöèE?pXûQïÑ?rPöèE?ïñ…¸ë!?p'Ëâm#>?\õþÇã-]?p'Ëâm#>?ïü‡ŒÉ?5~?uÆC>?;Ú;N?5~?uÆC>AGN4FGL J2325.4-3559¿ÃXN[éÇÀQmƒùdoÀ8ö¬Lú"–À<¯Ù`Y@›©ä'@á%Ie¥?¨dË܌ÞJ?Ç:`Nq@jG¾²í@\¥°ÔÏ¿ÓÝåC;>¿ÛêÆ}'s¿ä€!Î\¿ç1¦k94¿íRCÏb©C¿ïÿ¾ÿ"°AGNfsrq3FGL J2325.3-3557CTS 0490?ï®ÕÆ+?‰ð"¿a?"x
¤…ó*?‰ð"¿a?ïu£Ƕk?ª!Cè$Q?'K¥Qd ?ª!Cè$Q?ë'Eq×¼?©ˆSšÜÈ?ÿbê8¡?©ˆSšÜÈ?ïɸ¡­Ëf?hÆ<í ?{#¯HÈÕ?hÆ<í ?ï<0F(¦?¢(4ݚ^í?˜yð:ëJ?¢(4ݚ^í?í€]˜
ô?À8çI$?³ý>µã?À8çI$?éaàD˜X?´6æDм?Êxºíž¡?´6æDм?î>&VUø?˜ª>£þ¡?§šš €?˜ª>£þ¡AGN4FGL J2325.6+1644?åydM	ÀD¹Bá& À:º$?ziSÀ<ƒ»ðÜvŽ@ +Wdë¼ý?þÖ>J¾j3?Ãrµ)B©?«kÿœF·?æRm —d¶@vӉ)‰ç?ïý¢È6¿Éo8&&Z¿àqkè†f·¿âžüå™Lm¿ÁÍ=
!—¿ïþb †ˆEAGNbll3FGL J2325.6+1650NVSS J232538+164641?ïþâ‹ÐÙ!?6ÓÀí`µ?!×>г¨?6ÓÀí`µ?ï7á»?d‹^0ú5?`yH7Œ›?d‹^0ú5?ïí]×ݳ5?dð.‹×ý?b¢'ý1?dð.‹×ý?ïûû£qV&?&'¾a¶?@qúáÛ¼?&'¾a¶?ïþ[ÜHH?%wêòŠ,Ã?*N€z‡Æ?%wêòŠ,Ã?ï¶Ï<â?ˆY—Åá¤?'zLDw¹U?ˆY—Åá¤?ïëøÏÆ8?n¶¨œa?dáió8?n¶¨œa?ïôµÎGe?HAZ‰@ýÛ?V"csõŸš?HAZ‰@ýÛAGN4FGL J2325.7+1821¿Ëã¸.'ÀCþwÿuÀ:8(y›ÍQÀ<NÌܽ@Т=­	¹@ÃåZbL%?¶(™Ò#¤¿­w?ö:.?õeU	FП@	Cü ÍU?ïçǟ'UR¿äéŸìD¿è´áMK¿ã›ÔÝ<†™¿ëQ©A­?ڔ‰¤Ùé–AGNbcuMG1 J232550+1822?ïýf'Ü7?&Tì_op?4Ëj/Ö	?&Tì_op?ïïâl'pn?a'x8y¯Ì?`"‡.y?a'x8y¯Ì?ïä+¹ŸÑö?pFñ,l?kÔFv+ŠX?pFñ,l?ïø÷ê‡É?5K¦z
N?OÄ ZӀQ?5K¦z
N?ïü7Þ`Š?:t˜6R{?>AÒ¦ŒŽ?:t˜6R{?ïŸV
èU?´¶UéøÌ?~°Tûë­g?´¶UéøÌ?ïëb¬È?q·· ˜w?dæ(íÛ?q·· ˜w?ïÑçÀÌl?dV£¦¾ë?w{¿61Ð?dV£¦¾ëAGN4FGL J2326.2+0113¿ÙÄ"%ÀK'ËûµtÀ:ÄfõŸ<À<"Ýao†¡@ºø"æßÈ@ü¸oG¶?¿˜p_õš2¿wåh£M9©?¹¾|§ñK1@bÁ5"âP?ïÌ;ýÝ¿×ø¾BEtÔ¿ÝÇ-ügš¿ëö>¶4ž?s"Âïö"ê¿ÑÓwá¸íAGNbcuSDSS J232625.63+011208.6?ïÿ.dÓzw?UPiHª?3h{
R?UPiHª?ïði!à-/?c¡<¿8¼?_-¼,gÑC?c¡<¿8¼?ïç›Ñ4ï?püì¼A?hêdA?püì¼A?ïÿÙi	Ñ2>ã‹o¿Mp>óK'	ù*µ>ã‹o¿Mp?ïý«	³?2C~·UÕ?2§¸.^ä?2C~·UÕ?ﶋ=ƒ?!¢ä‡XÃ?']0½¤1?!¢ä‡XÃ?ï傣ˆÛ±?u‡g֋?j}\f¦.Ö?u‡g֋?ïÿ«þ×=?8P_{—µ?aÏï(Ÿ?8P_{—µAGN4FGL J2326.9-0201?Öã,O"<ãÀLàyåŸ+ªÀ:e^ɹòÕÀ<""ÍŸ@Þ~Ðëj@/FÄàoA?¾ŠÀÏ¿¤«@¹ûÜ?äöÞ¸1µ?þ$qÔ®˜"?ïInÞÛ¿å^m=ðüW¿çº•"<¿éøû^°¿Î)F Mgè¿äC¯'9+AGNrdgPKS 2324-02?ïûe2x'ü?7äŸÒ«?Bk6"êŸó?7äŸÒ«?ïäi(1Ö?rU߄,C"?k–€ªsRP?rU߄,C"?ïØ!Å´f?osÇ?Ÿž0?sï15âüî?osÇ?Ÿž0?ïï]hï`S?G ÜºŠ'??`¢–Ô&$?G ÜºŠ'??ïðÙ8ì8?UñâÎÉSª?^M&PÑ?UñâÎÉSª?ïyë¯ïz?–4Ö=½9'?ßB†'tÅ?–4Ö=½9'?ïŒM¨Q?Š(µyYè?Œù,™i‡©?Š(µyYè?ïg†i¢Ù?ƒÝ0ø'eß?"2ÝSÖâ?ƒÝ0ø'eßAGN4FGL J2327.3+4717¿±*dcŸ9À*h–š
Ø¡À:·V¥ÿªÀ<~¦ã@N´C%?ý÷})÷JO?͈ܲóݳ?͏¸š:Ô<?ýýI‡2ŽÉ@X;¯X¦?ïãĕƦB¿è¨Ö]š9ý¿Û"oH7Œ¿ß}…fÜ­ë¿ä± VL<ï¿ïýB äfœAGNbcuNVSS J232723+471601?ïøÊü ¶?@ÖòL÷åy?LÖh¿"§?@ÖòL÷åy?ïç³cš.?nv2Á†87?hýL]-?nv2Á†87?ïڑòcè»?pÖô+«z?r·Àýn?pÖô+«z?ïªòŸÉH?aõÂSƒ±?…CX?=Iæ?aõÂSƒ±?ïóýÂý°?UýÕ#ϐ?YÞå8o°?UýÕ#ϐ?$È{?£ÕÍs.˜?6Ǹ?£ÕÍs.˜?ï'BrÚ%?‡¨…er/#?‹¯crz¢²?‡¨…er/#?îµÞl:ˆ?ˆÜ*ކû¶?¤¢8ô'?ˆÜ*ކû¶AGN4FGL J2327.4+0444?è"
áóƒ#ÀJ"Ðå`BÀ:Øÿ€¾À<f"Xð\@ëâÈÇß@q…Æ}þ?ÃX"ÖĝS¿™."hƒ?ÍêñûÛX+@ùB·Š›?Æ3h7Kñ›¿å.·£oÜ1¿åÀBŠ3ö¿ãdŠž›¿ì4üa'¿ÈK4Ä,ëAGNbcuNVSS J232733+044740?ïûÌmg¯?J¿û«?@ÎJ°³uá?J¿û«?ïîæbJ"
?eÀ¥!çE?a"á³?eÀ¥!çE?ïß8.ðƒ`?y›~£'|K?pc藌ƒÆ?y›~£'|K?ïûÄ@®"H?'Ïm¢<¶g?@îü¢kÖP?'Ïm¢<¶g?ï÷'³×ÿ?O‡…§=¬?Pú˜Š—rt?O‡…§=¬?ï±Çgª€"?‰Ié)%ž?ƒŽ&—ô?‰Ié)%ž?ïì-@¼?qʘdò:H?cÒ¿^>?qʘdò:H?ïëcÅø?TÑuÅ&TÆ?dñœ*雹?TÑuÅ&TÆAGN4FGL J2327.5-3259¿ëßƛt)ÀQ½Œ¨À:·pÔ~qöÀ<­æcvÇÝ@ø4O'åJ@3fÿéYË?Ë:Ïç/O?Ȃ;òŸo?ú'(bõ˜ž@¶Œ½¾?ï.Ô>[/|¿ÝzX@ˆÜ2¿çU~¢u¿ée2`=W¿ð?ïÿãåîAGNbcuNVSS J232747-330130?ïô<êZëù?\pde1?W†*Ñ5Ï\?\pde1?ïëú?T\?m€ò'‹?dãÖ©#‹?m€ò'‹?ïzÔ=jªÕ?‡N‡ZNkx?¥xJŸo?‡N‡ZNkx?ïò¡Žwõ?Gb¬¬?Z½˜Ø†Æ?Gb¬¬?ï÷€1¾"ú?WM7@?Pÿ	[h?WM7@?ïW¢Mi·¡?£[å.•s?•¶Y¨CÕ?£[å.•s?ïô"jý¿?–Ë?Ø'áÖ?Ÿ¡{·Ç²%?–Ë?Ø'áÖ?ïµÛm	ÔÑ?s;ɑzW‡?'‰$¸»W¸?s;ɑzW‡AGN4FGL J2327.5+0939¿ïû{j×åÀGü£a™xÀ8¾®×ï?¾À;§:-ù7@w"ìá•@tõÅêZ|?©4'yì€?ÀV:ߤë²@'bØ<l˜@µÌCŽ¿Ê
2îà¿äõÿ 1#¿éŸ¿™£¿è™cé´d ¿í‹Î2JU¿ðAGNfsrq3FGL J2327.7+0941PKS 2325+093?ïù"'l??DF>yŸ•'?Iïd<Å¢?DF>yŸ•'?ïêQQ=³?hÊD"ƒÐ·?e®¯)¤ö?hÊD"ƒÐ·?ï«IÝø ì?€ŸíÔ)‰?…-ˆˆÖüò?€ŸíÔ)‰?ïýB?·óC?%›-@-:ß?5î…ªÑé?%›-@-:ß?ïøeÞ<r?Sp}«ÑNm?Nh† Dbî?Sp}«ÑNm?ï¤È§¬µ^?ŠD%誠?†ÍÖ"'y?ŠD%誠?ï´ñª/q?…ûÁiݸY?'Õcýr?…ûÁiݸY?ïóï/Ōß?P6˜ª??X! ö'r?P6˜ª?AGN4FGL J2328.3-4036¿è?ÌQZnÀQ
-à
qÀ8•t/|ÅMÀ;¤BW"dÌ@—);¸'Ù@©Cäõ?£–œÂ¡ƒQ?²½g4@H/yjO)@ǶãV|?Èd¤Yæü#¿ã²úÉ_Z¿å5¥Õ?¿ä%'(]í¿êÅ
á?¦¿áĆ!—ªVAGNfsrq3FGL J2328.4-4034PKS 2325-408?ïü&*o^?7cýíÿ*?>ήÃuš)?7cýíÿ*?ïödirE©?Wä¦X$÷_?S7-.²~?Wä¦X$÷_?ïË8™é9"?yCÎeÀ-?zc³%€E÷?yCÎeÀ-?ïÿ¡ªŠ-?E¥:|(È?KȚ"˜?E¥:|(È?ïûëIuÐù?=2\ÿ«=X?@RÚØ_M?=2\ÿ«=X?ïÛoÿ䞝?x3õâúœ?rGÿü'¥•?x3õâúœ?ï¬óþê×$?‡Á{˜n?"ÃS¦ó?‡Á{˜n?ïý-]~?/&v"ï?6—æ¼#s?/&v"ïAGN4FGL J2329.0+0832¿î˜ëme¢áÀHúÁҝÇÀ:X‰ÀßÀ;ú"õëª@	8BÆ¢@¡Ý»1™Ö?Ç/Úx±íx?"%îbYø€?ÆN³×³Z¶@ãçiܹ¿ã6|=鵿êMf»ü¿çµL»šu¿àJæ
²û¿åéázÙºò¿ðAGNfsrqPMN J2329+0834?ïýí©f@Q?#Ž'j¡Ð?0'³Ì´Tg?#Ž'j¡Ð?ïîu)*yY?e²çz£aP?aŠÖØFW?e²çz£aP?ïó'çŽÂ?]^"ÐHÕ?Y°1¯§,g?]^"ÐHÕ?ïû΋…?(½ä÷£Í?@ÅÓecÆj?(½ä÷£Í?ïý´)yb?+"°RÞ?2^²ÿŠœ?+"°RÞ?ï¯Sð³²?‹
¹Õ>Ú]?"+<5Á¢?‹
¹Õ>Ú]?ïê=x'ü@?p7j•?*Ú?e‡þ_ü?p7j•?*Ú?ïèéf>+?X¿z{´'×?g™óON7?X¿z{´'×AGN4FGL J2329.2+3755?ÒÐM\î»À6(ö¾7ޔÀ9œÏýÚÀ<ÂVQEm@ LêÇϸ?þ"]"<?±K£—tP_?Œ´íTy u?܉ݤ`r@"UZ$Ž«?ïÉÁ_[ZD¿â	€,A¿ã&pA±{8¿Ôúv=Éå¿Þ›‹Œ;¿Øp¹[UçAGNbll3FGL J2329.2+3754NVSS J232914+375414?ïý ä³ë¢?&â'Ø"£È?2øÙ&-ç?&â'Ø"£È?ïóf
Èaû?`C<Iíj?Y3䕷¨ö?`C<Iíj?ïöY[™Œa?[[­'´?SMI:Ú½?[[­'´?ïð|õt
ê?GM3«üš?_F¤ÜC?GM3«üš?ïûëIÿAX?4ð65?@R×Þ±ón?4ð65?ïËê™çGL?~n›y¾]?z
³›i½?~n›y¾]?ïò…U>÷?fÙ7¨†œ?[òõË´¡ð?fÙ7¨†œ?ïÞ¹µÝ‹Ñ?\éé´ØC?p£%	‹«?\éé´ØCAGN4FGL J2329.3-4955?àÝð-ŽsÀO'L Â'ÇÀ6×TûÚ×RÀ;A.jv–_@¾5°;@iÂÝ`?‡­ºÚôƒ?»֑ò†@,úuFÓùè@"ùÃǕ€¿›oðAµÆ»¿àe•P^½%¿äâb`Ght¿åšÅ都¿é°
Ÿ@L¡¿ïHG,{ÄAGNFSRQ3FGL J2329.3-4955PKS 2326-502?ïè[DZ‰?dàñ§ŒžL?g¤»…Úyy?dàñ§ŒžL?ïˑ©¸˜?‰žhíF˜T?z7x"4¸
?‰žhíF˜T?îŸÂ‡=eU?Ÿ)!˜sWO?¦׍'®?Ÿ)!˜sWO?ïú5KÍo?Sª‹¬ãw°?G"+Ý|ã?Sª‹¬ãw°?ïםÈtÅÇ?jbö¥Oc¢?t1°ÿt'?jbö¥Oc¢?ïÇT׌ˆ?¸Qî³,h?ž'^/7?¸Qî³,h?ï_0èÄá?'©zˆzÚ?"ìHÍÓ?'©zˆzÚ?ïÄT׃ñ"?€]¤úä?}Ք#:{'?€]¤úäAGN4FGL J2329.3-4733¿ëº'´óÃÀPÂÀð À:FM½"4ÞÀ<P!ÀD(N@íb ®ì@ä1æ,c?¿ËÜ!~ã?¥añÆ\Æ?âùåŸ+©Ò@:-1;ŒH?î>rο济¢o¬
¿æ—"[tšÝ¿âh>Õ¿ïÿªÅÝð¿ïü»!©ôAGNfsrq3FGL J2329.9-4734PKS 2326-477?ïü=ù4ß±?1·ÜuÞ®,?>8z^S?1·ÜuÞ®,?ïõç€ùB?WV÷/7UK?T1Ôèûv?WV÷/7UK?ïãTx¨2d?id""?l«‡d,4D?id""?ïý¬B›û?!]˜P±F?2ðHã2™?!]˜P±F?ïûƒ
®Q.?9Vp>ny?AóÔ^/R"?9Vp>ny?ïݘÝ*ç?vIxÕòv?q3'r›¸_?vIxÕòv?ïÞ4Ó8»?y-¼†m"Æ?påÀ0€ª ?y-¼†m"Æ?ïùX/…Ã?@Ûaˍ<?KšŸÅM4Þ?@Ûaˍ<AGN4FGL J2329.7+6101?ïÖ.²'[Y¿Ò׳ϝÀ9"å'–pÀ;Â`{jÚi@ ÷u½qe?ÿ9  ?½X¡VÒI¹?±½wg?ó·
1A@9úÄ+éh¿äÛQàG}î¿ÜÑT
H¿ä=Ýܽ¿ÔÐß´0¿äÒ÷S‰¿Þ=Á¬ˆ4AGNbcu3FGL J2329.8+6102NVSS J232938+610113?ïüõ›;ôè?a1ÐÑÎó"?8S%A%X?a1ÐÑÎó"?ïåô÷
h?sªÜÈz{?j	&ÑòB?sªÜÈz{?ïîÈGR?ppÙY<¥)?a7â²Æ?ppÙY<¥)?ïä»ÿ/p?T=µ'¯"?kDI¯|?T=µ'¯"?ïübH'??6ß-špJ??Ôîn²	-?6ß-špJ?ï ütt
?©+(¯?›ü lJÇ?©+(¯?ïãÿ99:<?x…
4ÑÖ?lÆÊåL?x…
4ÑÖ?ïŽTž™?{		ö1?ŒjøØ™¤?{		ö1AGN4FGL J2329.7-2118¿ÔûˆÿdñêÀQ âe+ÔÀ:ÚJcÑaÀ;홭»Ž@Ù"˜€•@¾0O‹Y?ÂÏ
¿¡–¿‹ã­'Ú©H?Èô{§ìÁ@ï¶wö±£?ï²ÌÛæED¿ë棣×e¿Õ§¢Æ¾ì¿éÍÛU%ÌB¿âQ7@¿ïù˜¨)AGNrdgPKS 2327-215?ïíG«²˜?e¥q_Üé?bã¸?¯¿â?e¥q_Üé?ïëÕL^cŸ?q¤íiAc?d*³gâñ‰?q¤íiAc?àÌZ?†]­×b‡?×‡Ú¸x?†]­×b‡?ïßÿ ô×?Y"VŽDa?poã¦ü®?Y"VŽDa?ïšÐ·y9¹?…†O
{?‰KÒb½Ò?…†O
{?ïÏ>;+?Ž,åýz‰?ˆŒ0s'ýV?Ž,åýz‰?îmVY Q¼?¢`Ä¥@?©*šij€;?¢`Ä¥@?ïq™ÚÔnÏ?a¶ˆý'ÿ?'ÌÄ¢Š#?a¶ˆý'ÿAGN4FGL J2330.2+7759?çu%'µ@X@/œŸ"…]¢À: ÝU±}À<]pŒZö@ý÷ºa:X@⿐¤(?½¦´4P?¾wðýX°Æ@@Äe?@
~åkT6ä¿ãïa·ªü˜¿æE¿ý±q¿ä•[Fw´¿ã‹B¸â¿è‰ýÅ=6¿ïý«Ç™‡%AGNbcuWN B2329.2+7743?ïû>ÞÑQ?Dû—ã"Þd?C‡_Ã|œ?Dû—ã"Þd?ïïk"'b‡?báÃ'ª7z?`"kCPÃ?báÃ'ª7z?ïèMăýü?k'—êž?g²;QfÜL?k'—êž?ïô´1öGE??¢·M qC?V—œŒc¶>??¢·M qC?ïá3n
ñþ?l´"Ü¥Â?n̑²Õ2Ø?l´"Ü¥Â?ïºoíÎ¥?‡õïTÍ0?d{€¥?‡õïTÍ0?ïÄï_bªß?"mZ±‡c?}ˆPZY<…?"mZ±‡c?ïÐÀë†?cßÝÿܺó?wŸøñªe?cßÝÿܺóAGN4FGL J2330.3-2332¿ÏQ¥ö/'áÀQÖ"t¼jÀ;t‡'YYÀ<¦ÞãOÆ@gÄW]_@p Ç`?Ò»ûS?¾P[!¹¹?îրÀ.Ù²@d.'Ü¿ïõúÐ7»?î;¼(ßó¿ç"€$þg¿Û#ð_£ÿy¿âý²}–-Ô¿ïÿ?…¦óAGNbcu2MASS J23301617-2336413?ïûÖ²ÿœ-?9çòàӝm?@¥3¡Z<¾?9çòàӝm?ïܙq^D·?~æjø…Y?q³GEÞäV?~æjø…Y?ïÒB•Pߖ?s•Þ¬þ».?vÞµFb(Ù?s•Þ¬þ».?ïåAL?b…?SÙlØBd:?j¾³ÿÖJ^?SÙlØBd:?ïöÕQ€¦.?V*´óe?RU]içt?V*´óe?ïqKëšß?™¸#€4Y(?'Ö'—Å:$?™¸#€4Y(?ï¢#êß?ˆ_9þ&ם?‡~w,ÆØM?ˆ_9þ&ם?ïoNø".~?"G­Á¬K»?' ëÂb9?"G­Á¬K»AGN4FGL J2330.3-2948?çbõ´ˆÄpÀQÿÐR"JËÀ;Ñx-8GÀ<Áû
Qø@`ŒŠ¸Ö@sgÁLf?»Ío4[\¿·–Õ™úèi?ú#=ó?è›$T"Lç?ïr-^ÝÛé¿â0¶¶àÒ=¿ä/?› '¿Ú©A­Iz¿Ûh¯a,Ü¿å&ÓßÅpAGNbllLEDA 3230048?ïíéMÈ?kû°zZ³Ü?b²b€
L?kû°zZ³Ü?î9Êüèô?»[Þý?Ë?®ŒcP1p»?»[Þý?Ë?ï]ÊíñØ?'·zèïç0?"\© üù?'·zèïç0?îü×÷ÉÍ?‰ËÛé¨Ù0? 2€‡|1?‰ËÛé¨Ù0?ïÙ:AMô?yK,éŠû?sbßrê¡Ö?yK,éŠû?á"B7˜?ÔãVÖ?V?Ü×{ÞÎÇ?ÔãVÖ?V?ïWjF^£?"îԋ<q'?•·4+£?"îԋ<q'?ææo¢Ç?»š8̋o›?Ò3 ºpå×?»š8̋o›AGN4FGL J2330.5+1102?ÖÝi	%eÀG‰c4'¾ŒÀ9úŸg8ô=À<¯#nš@ZV'©è@õNÂR ?Ç<5»MÉb?Ñ{Pw@ //˜t@
V¡¢Q¤¿Ô	 ØÅ¿çæáËâl¿ç\Á¡ö_¿îWšPx¾X¿ïÿÝÀåãÊ¿ïÿÿ)@k*AGNfsrq3FGL J2330.5+11044C +10.73?ï÷µ°?g8?R箐yÇÜ?P"Ÿe´°c?R箐yÇÜ?ïè³Â²'?i®¼ª	?gL=
™\?i®¼ª	?ïƒ"ŠL'T?…¾A ÷÷?7]i†"?…¾A ÷÷?ïßF[õô?W1•"i_?p\Ò`Vú/?W1•"i_?ïùƒvír4?I"NV,?Iò#ԑ^4?I"NV,?…€:¬?'aó©,?ŠÙžœ¹%?'aó©,?îâ&Uª+?—;A>¤õ?¡Ýš¥]G.?—;A>¤õ?ïN¡sÌ?‰‡_˼?œÖ+æо{?‰‡_˼AGN4FGL J2330.6-3726?·G¶£WÂæÀQ‡ ù	kºÀ:MµåçPÀ<=æë\@'"Æç@#¥™'¥?³çW'Žž¿±ÑÅÁ&¿?üûÅÃď@6càÐ÷?ïNË	~.¿ç	ÃÞ;µ
¿æu^¡ví¿åw¥[Zš¿ÙUÛ}¿ž¿çŠÄê€;ûAGNbll3FGL J2330.4-3726PKS 2327-376?ïþ9ÚtÞ­?.ðßXê¤?,bWB؎|?.ðßXê¤?ïðXÅ5v&?hôU6Ç?_Nv…St?hôU6Ç?ïáWNÒª?s·«é­w*?n¨~Á«v[?s·«é­w*?ïù'‰ÞCJ?3!S¢GO–?I¹Øu[<þ?3!S¢GO–?ïýٚĨ?/†$Ԃ\?13)mòÏ÷?/†$Ԃ\?ïÄí~âÍÚ?ˆ%Übµå|?}‰@‡¹Û?ˆ%Übµå|?ï˜õTçt?€4G€(K§?z1…7ÿ¢?€4G€(K§?ïɇ\øuê?o#¤
}¤k?{<Qmžð?o#¤
}¤kAGN4FGL J2331.0-2147?åf#µç­úÀQ¾5'Ì÷À90b°Ï@À;ª"Xð\@BÏæ\ÀË@v´âË;Ó?°y5 W?À³³á™b'@c™,ŒP@¹@ÓÚ³¿Û9Î¿Öï=Û,áà¿çñZëÞàÌ¿åW¢žzÿÑ¿ìÛªëÑtÒ¿ïÿyB=KAGNfsrq3FGL J2330.8-2144PMN J2331-2148?ïð¤Ð%ê?Yt³¾ÒÒ?^¶`¢qà?Yt³¾ÒÒ?ïë9a ƒï?w1so­DÄ?dƞ}¸¡I?w1so­DÄ?ïr'Ã-?'{zÚ?Ýñ´ÏT?'{zÚ?ïûpú,?-`A‹öûÃ?B<îó¼?-`A‹öûÃ?ïáä´Óg?i$ÐìW†Ä?nK&ñ8Ã?i$ÐìW†Ä?ï§xÍFD]?ŠÏ°îV¢?†!̤ Ï?ŠÏ°îV¢?îÈðŽà£?šCî"Qï?£p÷Š'×?šCî"Qï?ïéS÷V–Ã?ZUó|?f¬‡
%?ZUó|AGN4FGL J2331.1-1653?ÝØËG*zÂÀQ3y¦µÀ:êDrØ
À<G¥rë¯ç@¨+i:V=@
˅¤ð?ÔØ[
è'N?³
f
uú®?á"	¶@të¢%p¿ãT°',㎿ºcß½.8¿è7=^ZS^¿ìë»%_5¿ïþ®[È}³?ëUI°ÎjAGNbcuPKS 2328-172?ïÿgÛ >?¢rŒ^?ŠLO¦¢?¢rŒ^?ïïõ¡µÐe?a"ûUÈrÄ?`
^\
"X?a"ûUÈrÄ?ï¥ú$–.Í?ƒÓl÷îšB?†väà —?ƒÓl÷îšB?ïü3_RöÈ?+ÓÒß~?>e4lÂ?+ÓÒß~?ïÿ®ž/ø¹?@‹µð|?X^°p?@‹µð|?c"S?˜8ñr¥b?‡'7k@?˜8ñr¥b?ï­®pãS?…R>N4å?""c¼ÍW5?…R>N4å?ïÙK˜s?gшÐsøW?sZr-—,u?gшÐsøWAGN4FGL J2331.3-1558¿ïº™^`]ŽÀQᛐëÀ:¶ÇǪNÀ<TtûTŸ•@¥¶Ê,@ÐE AY?Ð6̤?®ÆßԈÐ?ÝW¸"Æ©r@
³‰‹"ƒ¿ÊöZlˆ¿ëyJ]¿ßUûļ2¿ê†^¾Ò8G¿á(&à>™™¿ïöÕ´ÒÛAGNfsrq2FGL J2331.8-1607PKS 2329-16?ïÿ´þW'?è˜Ç©ŠU?I^€xà?è˜Ç©ŠU?ïî‹üx)?eN{Öís?atVzvÆ?eN{Öís?ï㝝"»?r»ô@çG?lbb²'
?r»ô@çG?ïþxÏÛ±'?«î'MÓ[?(rÿåg¸?«î'MÓ[?ïþ½I:ö:?(½š­{[?$+jj pJ?(½š­{[?ï¨EçÉ[?ðš®ØË'?…î†g®s?ðš®ØË'?ï×nO؟-?zÊ|Òl×?tHØ ¥ ?zÊ|Òl×?ïùQFˆi_?@¢(ì¿_N?Jºæ1ê›Â?@¢(ì¿_NAGN4FGL J2331.5-0258?ëx®+eÎ*ÀM™ìòù‡À;m/®CuÀ<'Ô{ø@ §6…º?ú¹Ð¦v ï?Ó¿²ÝãJ"?Ш $ã1?ü@j‰
Ö@kù«R(Â?ïò6H'iI¿èßvBQ‰5¿Ì/¥ßøù|¿Ù(ë܇ç¿Ðki$Ü®A¿ïÿÿ" 5•AGNbcuGALEXASC J233112.94-030129.9?ïþJBï=æ?!æ°bXƳ?+[ÑÍ¥9ò?!æ°bXƳ?ïîÚ¾Ò?cµvuTL?a%à<}Î$?cµvuTL?ïÝêԟ©ÿ?poýO1Ҝ?q
•Èè0g?poýO1Ҝ?ïûe…&+I?-ÙË¥¤^:?BiênՃk?-ÙË¥¤^:?ïÿ.à#}?D—3,?úòï¶?D—3,?ï£RP?'|‡¤Ÿh-?‡:ëküÛç?'|‡¤Ÿh-?ïÝ/íÐS?xéŽh©ÝÃ?qh	—€?xéŽh©ÝÃ?ïóÒ>ͬ?O9ÓñdGÜ?X[ßÄ]&÷?O9ÓñdGÜAGN4FGL J2332.1-4118?ÕºîmÜQÀQÎþÖ4UÀ:ÇÑ;ÇVkÀ<{èxú½¡@ûs'
@݇»¢?γ$Z'hÐ?؆~ŸBP@¬}Cø}U@"E¬/ô¿îß´tç?îa{zÊ¡y¿Ú@H%©ˆ¿éeDþ6Ò$¿ïôZ 4"[?ï­¹¬^˜<AGNfsrqPKS 2329-415?ïԌÔå)?y—Ý u|?u¹•­¼¿K?y—Ý u|?︀ôÿhM?"Á
ÃÈ?ß¯OÖÝ?"Á
ÃÈ?íñûÃ/j&?šÅxʵþý?°p!èªpN?šÅxʵþý?ï'ÐLÅÅ?{J=8?‹‹ÿé^ò·?{J=8?ï\B«B°Ì?•NSÜ1Tó?"wª @ìs?•NSÜ1Tó?íòøhkà?½KÝ'|µw?°h?þtnû?½KÝ'|µw?ëaÿ¡MÝ?©"
ÀWÕq?Âxázȍ?©"
ÀWÕq?ìF—¡qÕ/?±3ê'ÃW&?½ËBôqV"?±3ê'ÃW&AGN4FGL J2333.4-0133¿Ïz~á²bÀM)¬îàóËÀ:¨Ó¶ËوÀ<	Äf̽³@¢PE½¤f@[›Äí{?Ð<}>šœ?ÊuqǬ?ú]­	¸æf@dõu|Y¿ïh;ibš?ée·ýä¿åž¸‡›jT¿ëŽäŸQi¿ã=ÓLKˆ¿ïÅ¡—ûAGNfsrqPKS B2330-017?ïû¤Lê®#?S ƒ¶âäi?AnÌ0þÇ\?S ƒ¶âäi?ïê=1J"?dRâZ
¡®?eÂÎ¥v½é?dRâZ
¡®?ï I¤ÂJE?'»‹*cR?‡í–¾?b¹?'»‹*cR?ïéåªûR?OëÇ¥1k,?fU¬¾`?OëÇ¥1k,?ïóV@ÿNª?drî‹kµ?YS}Ç©;ì?drî‹kµ?ïyY¢€…?˜`v 5ä?Ô˵$Ùa?˜`v 5ä?îGđâ7?¢:s;™±?«ƒ¶ßHÒ?¢:s;™±?ï(7~hÞ?*Ïtbv™?šù2ä??*Ïtbv™AGN4FGL J2334.2+0736¿æÀ!¿S£§ÀIGFýëRÊÀ::DŸlAÀ<3ßTŽÍŽ@}³Ö†´å@ŒÏ¡"c?»ñ~‡ðNÝ?°`u¶uY?í¹Å‰¬Ü@uu‹u•?ïÿyYˆ¿Ùjh~™Ž¿äƒÆÞ÷Ö¿ê${àK.Ò¿å'XýÈ[¿ïÿúŒ"¸'AGNfsrq3FGL J2334.1+0732TXS 2331+073?ïþÎ-¹»g?\$/K¤Þ?#"RR¡'?\$/K¤Þ?ï퐊¸fu?fÛðcMTä?bouX«Z?fÛðcMTä?ïå€f(M?møŽ˜ðÿ?jš
Ëêˆ?møŽ˜ðÿ?ïþHij·?Ûešpr¿?+yeÃ
'O?Ûešpr¿?ïþÝ|â¦?²LY=ƒ?"(5fRc?²LY=ƒ?ïµ^¯kpš?Š ǐ?'¨T&Û§?Š ǐ?ïÎáŽi©?|Ðiç)æ?x8µÝ«Å?|Ðiç)æ?ïüXà/ÄØ?.é–Ô‡íE?=8ÿ}£-?.é–Ô‡íEAGN4FGL J2334.8+1432¿åáاmåÀF1(bõ˜žÀ9|G6v¾À;ïXÒÿìµ@XjGFˆ?þl»o?®Ï†C.0ž?¶'Ëïت@æ¥×Û@;FY€¤Ö¿ÀFdé8¾8¿Äa¦ù~†™¿áéàÙÊQ¿Ü÷jU¥#¿Þ¦YÛéuO¿î$…á*ý°AGNbll3FGL J2334.8+1432NVSS J233453+143214?ïþø¦øÛQ?ج"Òf#? uz¿?ج"Òf#?ïîçÌ#ü×?aԑ
€–Ñ?a3ð Ñ?aԑ
€–Ñ?ïèSúº,?qvm!šõ.?g¬™ÓÏ?qvm!šõ.?ïÿæì*-?ßá:G*?C!àËí_?ßá:G*?ïþüÿy?¯_"dç? >î©"Ö?¯_"dç?ï¨')?':F\a©?…úƒvê?':F\a©?ïãRÕåÐ)?w_|[S	~?l­)ûóG2?w_|[S	~?ïýóË¿0­? õ[WXÈ>?0a¢<Zޓ? õ[WXÈ>AGN4FGL J2334.9-2346¿Ù'j;=ÀRÚøßzNÀ:$Ú¯ä^ºÀ<aJ©q}ò@ÎRв_Ž@ܹ>z?»)9à '›?ŸÐb¿¤Œ?à"´/Gh@®òÇ2Y?ᅴ÷Aë]¿è%5y^¯¿æª>,‹y¿äùw_Ýá¿ìxá=G3¿ÏüƒHÊI:AGNagn3FGL J2335.6-2342PKS 2331-240?ïûÔj?9Gf$5Áñ?@¯êÕ)?9Gf$5Áñ?ïìÒ
©`â?s'eQk=?c-òZ¾¦
?s'eQk=?ïáhÑ-bA?kíºkÀÕ2?n—.¹àŽ±?kíºkÀÕ2?ïõÕ
D7Ï?Bžïz9î?TUë*™#X?Bžïz9î?ïõ¨_sò°?TÞæu*|"?T¯A Y°V?TÞæu*|"?ï§3:‹ò?‰×m勵€?†31y­g˜?‰×m勵€?ïáÖÒ½°-?t»̉
?n)-–co?t»̉
?ïÛhfÏJ‰?bG?1~µ5?rKÌ|-ï›?bG?1~µ5AGN4FGL J2335.4-0128¿ìÎ셵ó(ÀME>>)0{À:\+ŒuĨÀ;öȋ­@]ú͑ë@	Þu?Ěº@ƒ'è?ÓÖX¼¯ž>@
tBâӟO@´r€s®?âUT€_὿ä‡"Ô@^•¿å°¤xí¿éëâ§)¥¿çç™!#¼¿ïõQ@9AGNfsrq3FGL J2335.1-0133PKS 2332-017?îø£5,eA?ÄsðÄ	? u̯Í`ç?ÄsðÄ	?ïäÕJRg4?t~ܕöه?k*µÆUü??t~ܕöه?ïN\"eU?'ÐZ…cø?œ64h"l?'ÐZ…cø?ïä•S8â?RÊW)"Ö?kj¬ÁžD?RÊW)"Ö?ïÌXV¿e—?" ¿ceԓ?yÓԛ}Àd?" ¿ceԓ?ï†!›õÙ$?""fñóð?Žw˜ôËFú?""fñóð?ì«öxPó?§£Ç…e//?º L?xh?§£Ç…e//?îí†
JÁD?'$Ý#þ?¡'Ÿ-ç ·?'$Ý#þAGN4FGL J2336.5-7622?è5jôQRÀCõ¦ZÀ:d"j]kìÀ<‡ó×ӑ@Ä%4ÂÕR@«ÈÛ¦"d?¼¸€uÂ`?"þcGÍõ?Ôà´`Dc\@¥¹z׿è7ŸS—Ø¿Ï"na‡"n¿â2/ýô¿å"~Z#¿ãÞó`4s$¿å"à\÷RAGNbll3FGL J2336.5-7620PMN J2336-7620?ïþo9HË÷?}ðÚö?)oº]¨?}ðÚö?ïöv#¾í?Vc¥ÝBèg?S¸¼C•?Vc¥ÝBèg?ïðšpÈÙ½?hI}Žkç?^˝5÷?hI}Žkç?ïþ8'ä:õ?Ǧ=w@ì?,våö<Ú?Ǧ=w@ì?ïû½$'‡?;/…ÔʊÄ?ApÈԒ?;/…ÔʊÄ?ïß
­êË?}°²i?pz¨útú£?}°²i?ïð7Ϋý¨?p÷üM³Z?_b‡p[?p÷üM³Z?ïúCà5Š?;ì×-±J>?Fó‹¼Í?;ì×-±J>AGN4FGL J2336.6+2356?ÖÑ7{ºÀAê]yЦÀ:'ã8IªÀ<}\ã/å¡@sòvŽ+@‹4*©ø?À¬Ëxº?°Ö‡X¤\?ñ´)¸`.>@'#uP5¿ïø
ñâ?ïÿ*'Š‰[¿å3¢Câ-¿â•"z›¨¿×Ⴜ]hç¿é؃""^ŸAGNbcu3FGL J2336.5+2356B2 2334+23?ïúÐïû6?k:¬"¯Á?D¿üQj?k:¬"¯Á?ïçä=µJÙ?m`ʯ^ýd?hÂ(Y'?m`ʯ^ýd?ïéÎD"z=?iŠ M§ü|?f1»Giû	?iŠ M§ü|?ïãÀÇ?S]-xÜO?l?àühˍ?S]-xÜO?ï÷^÷Ìš?F«Áÿ%r?QB!|?F«Áÿ%r?ï"*•—,?›œ»ß€ì?ŠõZÈi	?›œ»ß€ì?ïåBdò&?rƒ'¸®@?j½û׆ú?rƒ'¸®@?ïi/{îè?ƒµKë(?'Ú}Ù?ƒµKë(AGN4FGL J2336.6-4115?ïñRY­àÀQHÙŽuyÀ9—ÇÜ£¦À<$«:«Í@Ã×öv"\@»tÝøn;?±dáVÀ{?½Y(ÿíOh@	Sü¡¦®U@zßøx¢¿µ+Pæ¢`è¿ÝA3¼pQ¿åO°!Etÿ¿æГ€ÐÊÞ¿åWõT«S¿åOß;AGNfsrq3FGL J2336.5-4116PKS 2333-415?ïû"º?O3ø>–Ç?A®Yããu?O3ø>–Ç?ïöÏvN?W™‹Ÿ`y?Ra?Fª?W™‹Ÿ`y?ïÕҊÚl¦?zÙ·HƒŠå?uºwLÍ?zÙ·HƒŠå?ïÿt'Lî?gÖBqµ?mÛÈEŒ ?gÖBqµ?ïþ‰¼+?)ÿÓø8…?'ngÖ~e?)ÿÓø8…?ïÙ.Iq?z¥'"µ?shþ){9?z¥'"µ?ï³;lEV)?…žrÊ·n£?ƒ1$â£ÓÎ?…žrÊ·n£?ïþ<šÔÆÛ?!º˜¯Ò?,6P†2?!º˜¯ÒAGN4FGL J2336.9-5859?êÈm(f?iÀKÐ<³åuÀ;VÅÓ´G›À<Á ªšrÝ@/ª›õiy@¸™aeu¦?ÜÚ]-W§?Í·Ÿ©~+?çx˜˜Ú@X…ïBÃt¿ïª'ñ¶'!?îa«IQ¿å¡­>¼ÿ$¿ä¶+ÀÎð¿ïÿìêy…þ?î9æ@;YrAGNbcuPMN J2337-5901?ïîɌÙö4?>úÏ-?a6sjäa?>úÏ-?ïóü`°'O?a¼³×á?X?"Î`Ê?a¼³×á?ïJÃ"²?Š~¢=J†?–§›«e˖?Š~¢=J†?ïû¶‰‹ÑÒ?1IÐ	P?A%Ú¼\-?1IÐ	P?ïñ©Aœn?a'™qD?\­}¿#É?a'™qD?ï¿Ujë†K?Š3ºdå‰?€*¥4 M??Š3ºdå‰?î9(‹mª?›">m[?¬mwLž±_?›">m[?ïæø±#à?`•Ä2)‰ð?ioz×®?`•Ä2)‰ðAGN4FGL J2338.0-0230¿ë‡öÖ-ÊÀMàÐÜüŹÀ9/{T44»À<
ª}í@tÐ%Ǻ¿@¸t »ÌÊ?¬¾lô-u?«ж'L?üu`4=þ@yFCcA¿×Â;cÙCS¿ã6M½øô¿æTŒê^®¿çç¾Àš¿íäŠÄÀ§?ÆP²ŠMÈAGNfsrq3FGL J2338.1-0229PKS 2335-027?ïýé¹Ò/?"‡ÒµÚ˜î?0·k¼©£?"‡ÒµÚ˜î?ïðmÄ\C€?c–8ôº½Ü?_$w)<o^?c–8ôº½Ü?ïçÕã»@?duߖ+7«?h*è6aÈ;?duߖ+7«?ïþ¼¢Ìâá?×ìÔž?$5×gWj‡?×ìÔž?ïþ5ûD?$VØikæÏ?,®Q<:Vñ?$VØikæÏ?ﰀϯfq?†r™£Ÿ?ƒßÌu7Å?†r™£Ÿ?ïè¹}(?nâôœîu?gÿF¿P')?nâôœîu?ïü£{çúG?46ݎ;'Ò?:ä —3×?46ݎ;'ÒAGN4FGL J2338.1+0325¿Þqn¢u
nÀKX³!ž¶À:ÁêÃê¦À<AF¹!õ@…F/9T@óMAÒ2g?ËmÖݜӶ?Æ	ÃbÀ¿x?ûI·ôÎs–@6+™Þ¿íÀ.ž£ï‰?îjA¢a¿8¿çöLÃ'1¿å{î|Iý¿á©Šrµ)B¿ïÿýç!éAGNagnPKS 2335+03?ïø£¥A?Lrç8z€Å?Msä*s¥?Lrç8z€Å?ïßuÔv?v¬­Áól?pE"#Œf?v¬­Áól?ïÏ,­ ùº?q*íFÆ_4?xi©€C'?q*íFÆ_4?ï×4ß} 	?\
Æ´°"~?tePŽC•?\
Æ´°"~?ïÍxdi{?|ôjæß?yCÍÿ	²r?|ôjæß?ï3»;Tê¾?£háj
›ç?™ˆ˜šŠ:?£háj
›ç?î·´üîÊñ?œyŒ«AM?¤"°1Pó?œyŒ«AM?î‹B!sÔI?˜'Yaί¯?§KÝçæÔl?˜'Yaί¯AGN4FGL J2338.9+2124?èÍ5QÀC2¹^Zÿ*À:»ö»³ À<UCh4œÀ@_FrÖ@(è6ú?´r4ûµB—¿‹v±ÚzÉ?Ø&IaÉ@(Çí?)?ïÿ¢âîwA¿à"-F<$¿än$Öyù¿ÞpDAùJ¿ÙK"\Ðg¿Ýô½ÑâAGNbll3FGL J2339.0+2122RX J2338.8+2124?ïþ™ÉËá?ôxs?&ci/é,¢?ôxs?ïò¯"')Ê?]]S:=R?Z ÙTž«?]]S:=R?ïõ½Æ8wÚ?egn ²í?T"s—O[?egn ²í?ïû_J	Ï?*‹å
Çõ3?B'×ð4¨é?*‹å
Çõ3?ïþ6x{Ö?$'oð‡‡?,˜uÏßT¥?$'oð‡‡?ïÅ\-Rs•?'¹±oU?}QéVIZ?'¹±oU?ïôۉ›H?fRùÀ¦œ?VH헎À?fRùÀ¦œ?ïôŸÍmå?DGCÅ)zÛ?VÀe:3Xû?DGCÅ)zÛAGN4FGL J2339.2-7403¿²¢÷QGÕ³ÀE7~ŽÒÀ:—âà4‰À<yyRژ@X*"~&Ì?þ¤(hÔÕ°?¶äø½–xþ?¦Õç}¨!r?ð˜í×ßO†@o[¸7"l?ïé`ŒÝŸ¿âÕÛN¿àÜ<ÁÒGá¿ÛOBŒf¿ãy«ó8qa¿×À
6Ih)AGNbll3FGL J2338.7-74011RXS J233919.8-740439?ïþå"P"I?Þ-¢½˜?!­× ÄÊr?Þ-¢½˜?ïöÊ$À˜?Vb½Eåw?SÈkøwN¯?Vb½Eåw?ïù%±HŸ?U'\XÐa'?Ki;Õ÷çÉ?U'\XÐa'?ïúà<Úë?0w¦QÉ{¡?D/*A?0w¦QÉ{¡?ïþUoaüc?[À	ÊZœ?*©
Ø,®!?[À	ÊZœ?ïÛ+¸s,%?£ytø?rj#¬üю?£ytø?ïú0×›ˆ?P‡t3ɨ ?G<¢§wîû?P‡t3ɨ ?ïõ9öEìô?Cµà@ëf×?UŒ³87?Cµà@ëf×AGN4FGL J2339.3-2656¿ØÞ9õLÑHÀR}|o½'=À;oˆ"xÐÌÀ<Évú2`¥@í°°ŒzL@Wª¹|ð?Ïå5¤Q®s?Œ°'¿7á?¿ø¢~¶_@»©äÀ^?ïª9ú͑¿çôÉ_¿åÕ¾]ž@È¿Õß/»Y‡Ü¿äÉï•N±¿ïéõ!T¹kAGNbcuNVSS J233917-265638?ïþë'fïp?e./,د?!G׌CÇ·?e./,د?ïð# æak?eêìº…?_¸¾¹íÙ®?eêìº…?ïðk§»<Ï?ZÏE¶å"?_(°ñú¯?ZÏE¶å"?ïþf'?%–3!h?)—ÞۋË?%–3!h?ïÿPvB°?³"põ+?uö*M+†?³"põ+?晴õbP?aõ@óàï?…ÛB'hü-?aõ@óàï?ïÜ0ôÙJ"?|™ZÀ?q煢y6­?|™ZÀ?ïúè΂{è?9&µ@k|Ø?D\Å[f©?9&µ@k|ØAGN4FGL J2339.6+0242¿Ü—gÔêAlÀKÀ"`ÑÀ:$رÝ]>À<+ÉMì@¡ÑÖvï¡@GPܑeî?ÃMK7`êQ?É¿?#€c@ù«ó8qa@
£E±,?ïܨAÓ	'¿å~Âþ—Ë
¿ç¡]]SBG¿èÉv7]d¿ïø[#*¿ïü'«@‹AGNbcu3FGL J2338.7+0251CRATES J233930+024420?ïð…"-Q?Y9ÛSÝQœ?^õ»i\>â?Y9ÛSÝQœ?ïèׁÜ9?iìO`¡ˆ?g(æ®>O?iìO`¡ˆ?ïÂ0»x€^?w½ë"[3?~ç¢Zm<Ï?w½ë"[3?ïÀ<Ȫ Ÿ?d°"ü´™?᛻ݼ3?d°"ü´™?ïàÉé÷?qË è<pÈ?oì5õ¸q?qË è<pÈ?ïšäº1ó?Žß^.e?‰†ß1ó%?Žß^.e?îÕ¡²AÜ?š°¡î³Å?¢®…ã$A?š°¡î³Å?Š×¬?€ŸÛN±?§oô9æ:8?€ŸÛN±AGN4FGL J2340.5+3854?Ы²d°sÀ5ëVûW÷À:á½ñg·À<…üÉêš=@ Ih«»M?þó•:a%?Èîºu\N?©PÃß4к?äfg=%û<@1" k³?êÚÛé*Ñ¿ÇÀ[zO&"¿é´ò?øé`¿Ô°– ÀÕH¿Ï^c¸Œ¿êg%©ôçAGNbcu3FGL J2340.7+3847GALEXASC J234042.83+385510.7?ïýùƒË7]?'ðhœšT¨?03àZ7©£?'ðhœšT¨?ïð×Z3A?dg?0ïÅv?^QK–¾2T?dg?0ïÅv?ïð'pÍÙ?P%ñ2A¶2?^Û :½Ú?P%ñ2A¶2?ïõ¡«
~?9'ÑÄzc4?T¼©GSü?9'ÑÄzc4?ïüG†Þ/?>3ºt'ã?=ÃÐB¸•?>3ºt'ã?ïÉ2A¬ÙÎ?'Ë	==e£?{fßGϨ™?'Ë	==e£?ï슡rð§?mfUÿûË*?cu^È( x?mfUÿûË*?ïÓP.8?eìÔÂ'Ù?vWéÐ+œ?eìÔÂ'ÙAGN4FGL J2340.8+8015?좂^>¤«@1Ðx·¡Â]À8»ZôB\œÀ;œ—ü
§ú@ Øf3Í?ýmlš]
ø?¦/ºîí‰?·ø«wènê@Qš&‡S@uþÕ®Ë?ï¿t¿Å}M¿â¯LåÄ¿ÜÂ~_o׿ԈB#þÀ¿â\ʵ›X¿ÞR+[xv´AGNbll3FGL J2340.7+80161RXS J234051.4+801513?ïí)"f_8?\œ2‰•Ä'?bÖ{¶}±?\œ2‰•Ä'?îÊý{… U?ªÂ'\"H?£P(G­ú¶?ªÂ'\"H?ï¡àG}íí?ˆkt*9Þu?‡‡î5°î?ˆkt*9Þu?ídH1¥?•b[èÿ n?·4ݽ(ø™?•b[èÿ n?ïÄxOœöE?{ýº—g?}ÃØCbÕ1?{ýº—g?éI»r(Þ¾?̒Ê=Y?ÊÙ7\…	?̒Ê=Y?ïQò"Ç«?"ãΓmÒä?•ß¡»§
›?"ãΓmÒä?ãÏWâÑ,>?´Õ±4ÜNÍ?ØaP:]§"?´Õ±4ÜNÍAGN4FGL J2341.8-2917¿ØžeáØ£ÀR¡quŽ!–À:öä/À<±páêkC@~¯—ݬÄ@ۀ©Þ‹;?Ìs‹èÖî?Àx)Çόñ?ñàV·œ¹à?ü¢òÙPé§?î³àֆ¿Ó¬p¡RË¿ágž	jâÍ¿âBl¡"ãø¿ïÿF!!Ä?ïù‹a~ÖAGNrdgPKS 2338-295?ïÙBÛ*ä?s^P꿁)?s^'˜W©ý?s^P꿁)?ï»ažG?"'jy…!ô?~¢O-Œ@›?"'jy…!ô?î×j÷
R?"Y¯ÆBR?¢‰P#CÞ?"Y¯ÆBR?ﮄ¼"Ú?oyA¹äA?"^ÐÏ̕Ÿ?oyA¹äA?Çu?‰¢/ß#Ž?ŽÎ&'×Á?‰¢/ß#Ž?ît<ŽŒÜX?·™.囥¸?¨¼7Åï{?·™.囥¸?îÑG£á#Ï?™Á›o¨Ú?¢ë…¿Z
?™Á›o¨Ú?î!Ýðá?Ÿn½4ïÅ?­â ïTZL?Ÿn½4ïÅAGN4FGL J2343.6+3438?ê/'¼³O"À:.o`àëhÀ:+'›O|À<>9E›ëƒ@ á{´×7µ?û=uâlv?º…™\‡ëF?°ZKÐãݵ?ö T3]û^@Lï‹h©b¿ïԍöÎ(?ê`=X¿ÂÝÚ%ÐÊ¿Öe
{"Ý¿ÞÝh»Ö/w¿ÅWÙc¯AGNbll3FGL J2343.7+34371RXS J234332.5+343957?ïÿL^Rp»?
 ´î2hÚ?t3Œ'Ú?
 ´î2hÚ?ïñJffÍ{?_ÙSgÃ?]k2Ì°›1?_ÙSgÃ?ïö61❑?\
[¬Û·?S"›¼S>×?\
[¬Û·?ïø¾H¥‹?5øktqk`?OµރL›?5øktqk`?ïþð…†»?'^n-? ÷§ÚÓý²?'^n-?ïțtæ?…,¥C\¨?{²Et?Î:?…,¥C\¨?ï÷T³FÐ?d߽לÎ?QçV;ýy?d߽לÎ?ï힞2§ê?R2äóÐíÒ?baaß6
†?R2äóÐíÒAGN4FGL J2343.7-5624?î'ÜqÀM(6CˆëÌÀ:Íã˜Á,†À< †TBw@Â>%Õ|Ÿ@ç<º›qá?ÀÊ¶Ú ¿–rŸj`h?Ôì¾Ü-"@Uf¤S1?¼æ+ÿžlx¿ç¶Â3얗¿éÌVè'¿Ô¼Ì¤ˆàå¿í=Û,áàZ¿ãYyMÉ·oAGNbcuPKS 2340-567?ïýï²ÆD?%B/ÇÌÏ?0"Îõ'Õ?%B/ÇÌÏ?ï÷‰%¥xl?S''"þÖ?Pí´Ÿ§??S''"þÖ?ïêW5¾J?`²Ø¼è{Æ?eb¨ýío?`²Ø¼è{Æ?ïÿcYãît?ŸûVÇàì?"Ä4Á
ˆ?ŸûVÇàì?ïýZU®T´?1ˍ5xÿ?5-QLK®l?1ˍ5xÿ?ïݛ
Õ=?rRéøÿË?q2z _ÿk?rRéøÿË?ïäËc7ª3?un*¬QH?k4œ³¸%a?un*¬QH?ïý¶ý¶,U?&fò+Α-?2Hõß?&fò+Α-AGN4FGL J2343.9+0546?ïzéîEÃYÀJ¢pCßÀ:ª¶P‰…OÀ<iDo›™N@…Ã÷¼º@%`â˜ç?ē['÷
é?Ò­Ûzº†N@	»ž ç×@J¨;rò¼¿ëoyȸ?ѼB¦m½s¿ã
,kü¿Øò.Ü"¿éΕßе¿ïÿëÞ
òAGNbcu3FGL J2344.4+05491RXS J234354.4+054713?ï^ðZ	z—?"£•Œgٍ?"!ôůå?"£•Œgٍ?ïj­¤'E?—ávB 8?'¼jRNïa?—ávB 8?î¸!•.®r?—Éê?¤}æ®Ìæá?—Éê?ï5¸Që…?yÔ&A5?™\(úéùU?yÔ&A5?ëtv¥ßß4?½7Ò$t?Â.%h€ƒ.?½7Ò$t?ëÿмgò?Â+ÿˆòé}?Àð½`7?Â+ÿˆòé}?éòqw?µPœ5 ä?˅È6:#½?µPœ5 ä?êC±ÒÌ@?±8ÛDzÙ?Æñ;Ì´Îÿ?±8ÛDzÙAGN4FGL J2345.2-1555¿î˜æ
¶g[ÀQ¿j@»À7!–5dfÀ:þO'åJr@Þ_ùÎj@E}àÖo
?'àQ—ì}?ºW±þÑgø@&§lH'¶þ@ª#
¡S¿Ç¼€xá¿Ùòì;}·¿â_Ï=ÀTï¿â?êÁf½¿çø@îݘͿ糝쏋AGNFSRQ3FGL J2345.2-1554PMN J2345-1555?ïñƒÙÅ.?XÏx*¸€/?\øĺi#Ù?XÏx*¸€/?ï¯òc?–[Øyña?"?f3&?–[Øyña?ïF–3ÕçË?–Ò¦˜•?—-9Šjpš?–Ò¦˜•?ïóø%Ò2Î?Z ò›>èz?X´'âÅ?Z ò›>èz?ïæe|†Ž?gGë›m§?i皷³h?gGë›m§?î¶Wᤆn?¹Àaõâr?¤šæ"€"?¹Àaõâr?ï¬L'‡Á?‰ë´->ˆ™?"ìö+ùŸ?‰ë´->ˆ™?層g—
k?ç¯Ò–g?…Ñ&+kqF?ç¯Ò–gAGN4FGL J2346.7+0705¿ÇÍ´Ô2œµÀJ.XOLnnÀ9,¨hiuåÀ;Ð֟´eÎ@ 51¯=?ýŽ Ç‹Dl?­-=¿—ôÃ?–oBᄝg?ìHÆxõ@íÈs÷žˆ¿ïÿíUÙPi?ïþÝöÀ¼¿âðûµîcö¿Ñ	ç_u0"¿ã£—I]A$¿¾_ðÀòÎêAGNbll3FGL J2346.7+0705TXS 2344+068?ïþŠ3H? 'îkí¾"?'_àʔBß? 'îkí¾"?ïíDÀ4Ÿ*?e1=$y¸"?b»?π]Â?e1=$y¸"?ïÚr§hË?zBãåÐ?rÆ·Ž¾ö~?zBãåÐ?ïéz}¨*	?UÌý˜ûÛ?f…'GW×Q?UÌý˜ûÛ?ïù*áË?PöÇVõõ?JSÿk³?PöÇVõõ?ï±øA‰|?‰£¼4£å?ƒï¢prü?‰£¼4£å?ïÃ
.E$?"Œ'"d=§?~zèúùË?"Œ'"d=§?ïÆþ>£™?uë	%Q?|øӟ¯Ê?uë	%QAGN4FGL J2346.7+8008?èØÀ®[r—@1 -à
À9º¶åÚºÌÀ;ÍÂ5fê@¦7Õ.p+@…³ƒO«9?»(
æª?ÂK²›s8‡@iS×@úȗ^¿ïÿÀ_V&Ó?ïÿHkÇÏ¿äçøé
¿å÷BÂo¢¿èy‹!0Ò0¿ïþõÎÇúAGNbllWN B2344.2+7951?ïí"Ëh7'?p ¶^ÄW?bl4Òá·?p ¶^ÄW?ï\¯¬¼;?›¾2%"@ ?"j
kÛô?›¾2%"@ ?ïqۃ¸ Š?ŒèÓSÿ¥u?'ď‡4 Ë?ŒèÓSÿ¥u?îгÿð?€ý¦<tå?¢ôÀíJÑ?€ý¦<tå?ìf,†é
=?À6B$pU[?¼Î›È·®?À6B$pU[?ìah@u?Ä©4½Þ»?¿Ìô¿üY?Ä©4½Þ»?뒙Å/ìÏ?³Ú 4W?Áµ˜ë@LÄ?³Ú 4W?æ—MvLÚÇ?·8ŽÒä?ÒÑefJs?·8ŽÒäAGN4FGL J2347.0+5141?ïJñ=D"À#Ԕ-IgÀ8* Á@§À;h$Ÿòy@EY,ìó?ûñ«#.Ù1?lÊ{QE?¢µê!
Uˆ@TÀ%@hbå}rÇ?ïÿ5À+SÁ¿ºcCÇ* ¿×j[h†|¿Úï ^Å2O¿à
͞ƒä&¿×*kÄR{AGNbll3FGL J2347.0+51421ES 2344+514?ïþÈ{•ˆÏ?/^ÈO…¥?#xFÝöy?/^ÈO…¥?ïò7½}ò?``¸Þs?Zߐz\?``¸Þs?ïÙ¬ìݎf?y½üß"?s)‰x{?y½üß"?ïîü#ÉÖ?NìÖy·ZÒ?aÜNç?NìÖy·ZÒ?ïý°jŸ
Õ?-{²™×Q?2|«ø\Z&?-{²™×Q?ï² n_"?šëªè´O?ƒwägo??šëªè´O?ïÑþÏB6Ë?oI¼Eã?w˜qr~c?oI¼Eã?ïæÚìŽøÆ?Yå£6Ìz?i%`‰"?Yå£6ÌzAGN4FGL J2347.9+5436?é'ÂŽõ®Àƒ#5.À::sí7¦_À<4¨ÒÁ'@!†Š!×k?ù?yB=K?¾%ŸÌ¹–?È'?Š¤z@ÁvÂÔüF@RbŸ\|-¿ïÿéÅ+Ü?ï÷‰8ùEÒ?ꝡ»üñ¿ÔŸ4£ ®Œ¿×ՙd•€Û¿×n:%âeAGNbcu3FGL J2347.9+5436NVSS J234753+543627?ïßBßN…?q°ÕR?p^±øå³?q°ÕR?ïÂÚËhÌ?Œ™i´SÎ?~'šQpz,?Œ™i´SÎ?ï¼êˆŽHG?~ø^aqí?€Å]Ì÷°t?~ø^aqí?ïnOÒ-èN?x—kù™¥«?'6¿j`1?x—kù™¥«?ïœÍ;e9s?ˆ{ÂÜŸW?ˆÌ±#B3?ˆ{ÂÜŸW?îè͇)L?¯t¶»\o¿?¡Ó#AèG?¯t¶»\o¿?î×Ò¬àž;?œL‡¿¾§?¢'Õ1öQ?œL‡¿¾§?î-‰‰ÛN?œyAK" ?­'gorK?œyAK" AGN4FGL J2348.0-1630¿íBg‡è[
ÀQù2‹m†ìÀ82Îí8}À;]«›úœê@ݾ•Q‹c@QþÍ?¹? ãò¿`ä­?­H­Bî½
@T¿Z'È@Ïîq¸)'¿ÊÊ«õ¼°¿à.‡'?àÁ¿å&ŸÔœ$¿äì~ÃÕW¿è%Ë5ó×Ô¿é™ÝŒ7±AGNfsrq3FGL J2348.0-1630PKS 2345-16?ïþ7y¥º?!5)`oœ€?,ˆe¸Ôð?!5)`oœ€?ïð£vg:w?b§ù=% ?^¹‰ó?b§ù=% ?ïâF+æì;?scòýóg?m¹Ô¶lÆ?scòýóg?ïÿ¤YªÚù>þ5·!ͳ?é §â;'>þ5·!ͳ?ïýw°Kô?1×) *aÄ?7üAŠ¢hã?1×) *aÄ?ï®&D&9?dˆ²ïë†?"~örf
¡?dˆ²ïë†?ïŌ^š/?€å*ý‡½=?}9иÂU?€å*ý‡½=?ïÿmÎ1Q?	'ŽÅ‹IG?F@Vf+É?	'ŽÅ‹IGAGN4FGL J2348.1-4934?í
*¦OhÀPlvJßøÀ;,ägô À<¨¦¹<Í@‹>âéÅ?ý‡RÀ—4?ÞKþzÄÂ?åՏHÝ¿c@úÆ[¯S@	M/ê©V¦¿éf™£U¿äÀóEšN¿ånç´¯ ¿íc¯!–'Ê¿ïý³¿µ?ïûžaTƒ»AGNbcuPKS 2346-498?ïþa²w‹þ?LüÁ+í˜?)äԏMDÑ?LüÁ+í˜?ïõPøÒƒ?YwƒDš›?U^yý‰d?YwƒDš›?ï0P¨&‰?¯äjÀkª?™õêüƒ`Ø?¯äjÀkª?ïûÑ´µv;?4s‹ACÐ?@¹-–t[c?4s‹ACÐ?ïýëSSAÏ?FgÀ; C"?0¥g9<e ?FgÀ; C"?ïÒ*YÅÄ?}±Œ£ãŽ?vêÓ*,vó?}±Œ£ãŽ?ï.¾ÿÖ:?'YŒûÜ?š(<à8Ï?'YŒûÜ?ïèr,É?hZW‡vçs?gÔ'ÄÆ?hZW‡vçsAGN4FGL J2348.3-6049¿Û"P{\[ÀKT¼M"ÉÀ;¼ZÔ–À=»µMTG@lR
¾Ú?ùžõ#-+²?ÞTñÿŒ<º?ÜÊ¡yaë­?ùã÷aËÍ@氛"Äÿã\ܯ˜ß_¿íQ±k뿸4Àüßå¿áõN€ìy¿àÓnÝ-m!¿ïÿ:=°AGNbcuPKS 2345-611?ïúÛÊ°V¹?:å'ͧš?DÔk‰é?:å'ͧš?ïö}+5+?TZc¥v.¡?S©R
q?TZc¥v.¡?ï";òېp?‡q<Á,?Žñ7íØ
?‡q<Á,?ïü-';¦l?)öSΓT‰?>"îv\»š?)öSΓT‰?ïùˆf/Mº?N)WT·?IÞgÁ:¶u?N)WT·?ïØ
Ìáˆ?€×øU¬?sùqï@?€×øU¬?ïe²œtë9?×?¦åÛ²?"I¬mòüÖ?×?¦åÛ²?ïô¤­§v/?P½9‰N?V¶¤¾Ò{?P½9‰NAGN4FGL J2349.2+4535?ÿ1
"FÀ/ÒmÚÎîÀ:¥ub'¬À<
È°ÞZ@—"Òã]@"Âqÿø?°yÅhÕW?²öwÁ½o?ñ/N6ĸ+@
ªúý·¦J¿Ðõ"¡•'w¿áþ˜h¿äÊæ¾:Å¿âz?+Žú¿Õ£'{šÖ¿ïÿX¥³ƒPAGNbcuTXS 2346+453?ïþÿã-??qì<¬Ä²? ɼs¤˜?qì<¬Ä²?ïöPÁäfq?V‰LcԐ?S^|G±<÷?V‰LcԐ?ïø0aWïç?=QhB™þî?O>{•qN{?=QhB™þî?ïþõ¤"ÿ?Ç#$ï*? ¥»ƒ&Ð?Ç#$ï*?ïÿ
㎡?áJ®äƒ?£›ly?áJ®äƒ?ïÊØÎ/DÞ?"ÎŽžôb?z"˜ï<Ⱥ?"ÎŽžôb?ï÷¾÷]UW?b‰†9]?P'2'e?b‰†9]?ïü³Þz…h?,´"‹ø?:aí(©¡?,´"‹øAGN4FGL J2349.4+0534¿ÈN(yhCÀKo?Rü&À:`%t-ÏFÀ<KÏå†6@¡-g—>@ÕÓ;{×?¼ÿØè¹èD¿"©*±.‹¯?Ö%Â1hWØ@	â²r®?ïV%;"뽿éàp]‹ …¿ãßvó|d¿æwÿëÞ
¿ç…æ>7ô
¿ïÿÓ?,» AGNfsrqTXS 2346+052?ïþVz¾•°?TÜ©Æ|?*˜SkæÊ?TÜ©Æ|?ïðÓªûÛ?aŸgyäÚú?^YԆLYN?aŸgyäÚú?ïñ¢Gpµ}?WPíê›>?\»p¨buó?WPíê›>?ïûBg>ä¨?,NÕ‰?BöcÓ"©æ?,NÕ‰?ïýT"×±?2úF‰?5[\A†$R?2úF‰?ï¾,óý6?…ÄyšŠU:?€tÃ*ˆ}?…ÄyšŠU:?ïì«"iG¨?kÃhÞÝcÒ?cTÝ¡·?kÃhÞÝcÒ?ïñì.UÃ?KRŽC?]Ê'V];9?KRŽCAGN4FGL J2350.6-3005¿Û¶(pŒ…ÀSA5Tu£À:#5'Ì÷À<k‰öŽg6@ÙZÂC[õ?ÿÅ%Ù®\Ÿ?¹U%¡OE? ¯&ɘdæ?ç?–¹‰$@\ü؃9[¿éµ³áC|W¿ßè|U»ô7¿ã×jµ€€¿Ù½Ü¡u0¿âf˱CÚJ¿Û²Ø
€ÇAGNbll3FGL J2350.4-3004LEDA 3231681?ïþÊ]63?‹Â)¶'?#^Š*iÖ}?‹Â)¶'?ïî48õGž?hÞù­{å?aËÇ>òqá?hÞù­{å?ïôs±lbî?R§0XQî'?W«+"R?R§0XQî'?ïþa=÷K??ߏÎbµ?)ì$Û2ƒ?ߏÎbµ?ïþ^£'ô?"Žì¼Tpo?*ïW¶?"Žì¼Tpo?ï"T*F?'³í>£ò?‹*õqè—Ý?'³í>£ò?ïôšô¸y.?b²:ÞKòì?VÊ`RôÄ?b²:ÞKòì?ïü[/H"?1¨Œ¨•/u?=&…UþG[?1¨Œ¨•/uAGN4FGL J2350.9-1416¿ïý²àJÀQ»y(àÉÚÀ;lmî$nÀ<ÉÎ	îü@]šÖZ•"?û6*^x[[?἖S"ûË?ÜH$".q?ù/H!×Á@~DÖHÌ¿ïÏBÈÒlI?ïòX!ªÍ¿ÛïY—Œ¿á\à
—2·¿â ¾z#³¿ïÿ>9 ²þAGNbcuNVSS J235111-141557?ïõ€ÍÅÆ?U0&"Ócp?Tþd'|…´?U0&"Ócp?ïلŽ³°?'\D'p?s=¹b·³?'\D'p?ïOËá%°z?ŒÁU¸RÉ?–ƒÝ¾À?ŒÁU¸RÉ?ïШxss?a*¬ôæ¬}?w«ÃÖ²\?a*¬ôæ¬}?ïà
–©F­?pmSk;%.?oõiF;2ç?pmSk;%.?ï\¥M_|?œ!NBþä?"kP,¦'?œ!NBþä?îâDë¹Ä?–ă¼³[)?¡ßû³Ø·?–ă¼³[)?ïGÞ ¹?ŠK\q[g#?—?»èà?ŠK\q[g#AGN4FGL J2351.3-7559?ïYŽß¯ÀDJ­ÕÀ­À:G,å;YÀ<d»±òUó@ iÐ~25?üµY~ —O?¸É­6Ú]?» ç¬!0§@HIёX@ØÔ2Ü?îöúÓpTý¿â¸§z¡‡¿ÑQÐb©~¿Þџše¿áú@¨f¼¿áz螺jÊAGNbll3FGL J2351.9-7601SUMSS J235115-760012?ïÿ‡m?7ÿc%h?oåwLŽ?7ÿc%h?ïõmóM•	?Wêq¤»<S?U$NØm¦?Wêq¤»<S?ï÷ÓÂpŽš?[¦ì'Ž¼?PX{)q†?[¦ì'Ž¼?ïñQš+;?Ci‹gÊð?]\˸p¹l?Ci‹gÊð?ïþt‰-ªw?!}Ü¡/ñ<?(·p'?!}Ü¡/ñ<?ïÜu®Ë|?sÕùDš¦Ä?qÅ(çâ?sÕùDš¦Ä?ïú²šá?U(™¨•-?G÷ݏ0±%?U(™¨•-?ïØÓ.¡å)?`ãx=†ü½?s–hŸ?7±?`ãx=†ü½AGN4FGL J2352.0+1750¿ï¢ò'røŠÀEd9¼º0À:¤Ó‰pÀ<\Ti
à"@T6üÁ\+?ÿ:F"bH?¼'uÆ«¡?ÀÚ™Z"†@gMú^ÖO@DVä"=	¿æK¿[o'¿áK+­,ôU¿à'ÉEnŸ¿ÚwPCKã¿éø@îݙ¿è,ì\µ½AGNbll3FGL J2352.0+1752CLASS J2352+1749?ïý¹AS?+þ¦úNŠ%?27åêi¦?+þ¦úNŠ%?ïîÈ´˜p?f[pwç	?a7á1Jˆ4?f[pwç	?ï뒯¼èö?eü¿6ÁÈ	?dmP‡Ï90?eü¿6ÁÈ	?ïö"; Xê?:@áx)ê?Rو\Yl?:@áx)ê?ïòSˆA?Uö=Ÿ?[YïBj1?Uö=Ÿ?￶öï¢?évLG·;?€BCç¡h?évLG·;?ï´[N%õ?"°4Ç¥?'é?äç^À?"°4Ç¥?ïáªf4V8?[cÁYÊÌ??nU™Ü'è5?[cÁYÊÌ?AGN4FGL J2352.9+3031?¼Ÿº@¿IÀ>®˜¹ZÀ;RƒZ'ôÀ<‡˜(€QÊ@¿§·¿tu@íx:¤?·Êóìn~¿¾\€^Š$@…ƒb°@È>¸w€??ïPz¼¿çwåê«%¿ä´þ¤á ¿ä0]ºpT¿è{~@w¿T¿ðAGNbcuMG3 J235254+3030?ïþC핚1?#®áăO?+Á$»ûŠ?#®áăO?ïáw¯þ?tYpP¡`i?nˆPÿžq ?tYpP¡`i?ïãÍF'¬2?uŠ_Žȯ?l2¹v'Þ0?uŠ_Žȯ?ïÚ<¹·É?[ڍø¢"à?rᣅd?[ڍø¢"à?ïñ§ál'W?bCÜ­¦P?\°=$ñ¢?bCÜ­¦P?ïs',%Þó?™"sÞN°?'º€k‹™?™"sÞN°?ï—0>CÄ?\ ¬ø?Š3þpo?\ ¬ø?î™V©ÁE?•ÀWž?¦j•b6ݶ?•ÀWžAGN4FGL J2353.1-4806?çxꔀLŽÀP‰VC´À:ÉÝÑôÀ<Å
?#@L£Ór¦@$É Èb?ô2â€hE?Á>Áh¼,?ü\e¬,CU@Oš"Ñ
Ÿ?ìÕ©ë të?·˜Jd°¿âzé«)äÖ¿Ü|Tú®1¿å`ºŠªéM¿âB¨@ÑVtAGNbcu3FGL J2353.3-48052MASS J23531112-4806045?ïý¨Ž÷Kž?$ë<—2b?2»‰_©>?$ë<—2b?ïò˜uúz?[¶BÛ;Œ?[ÞÏ7ÆúÖ?[¶BÛ;Œ?ïñq—ûgs?dµÂ4d€ô?]Ïåu+ ?dµÂ4d€ô?ïð½‡+û(?C(ül…`é?^"ñìÁß´?C(ül…`é?ïôªý¢¶+?Q-ê`ë?Vª推Æ?Q-ê`ë?ïÑáñÄu]?€¸‡"‹?w6'{?€¸‡"‹?ïç.jv–_?u¢˜
kEv?hѕœ§p"?u¢˜
kEv?ïËß-Ü?hÜb
ˆ¡?~:|	õÒ?hÜb
ˆ¡AGN4FGL J2353.5+6646¿à½",Asà@&QßƤ•À9ëîÑÀ;'F1<¸î@½¡†øØ@õçB™Ø"?ÇéÀãàd¯?§ðd+´Ë?ã—cßM'ë@Áûa4Î>?ïþùÛ"Ðå¿Ùÿ€>Sοí5{!‰g¿ã^«‡ça¿é ÝZ¹‰ú¿Ô6ŽûçAGNbcu3FGL J2353.3+6639NVSS J235301+664243?ïàØ ×ª»?~J×5y¾?o'ß&õlé?~J×5y¾?ïÔlÀêã±?|r¢¬Œ>S?uɟz¿óÐ?|r¢¬Œ>S?îÃ<ÕP4?–i÷‡¹Ý?£Ì2±Î±¹?–i÷‡¹Ý?ï«Ga=‡ ?fFTÚÄ"?….'¦OD?fFTÚÄ"?î‹àÀÁóø?©n~"ÒÜç?§Aóðq$'?©n~"ÒÜç?î'!€XU?¯ƒ¹}L¢i?¦íçýdñ?¯ƒ¹}L¢i?ëfQ¸Ñ»?­Ï*È?Âg²¹¹?­Ï*È?ì¨{U"\?¢çáY¯p\?º¼%Wí"?¢çáY¯p\AGN4FGL J2353.5-1457¿ïÉœ×¢ÐÀQö¨~8ëÀ;DâΖÑhÀ<Ÿþ­©@ (&VÉ@íÅjؼ?ŧRiÚ9G¿­eyxù?çþ)f*×D@÷»õ9'"?ïîX¾7,¿áËހ("Y¿êà*b)?ê¿Þ"aùð†¿¹ n†,¿ïÿÀéz-AGNbll1REX J235320-1458.9?ïúèk0G?@FÐýà??D^R4ÎÆ+?@FÐýà??ïêÝøiS?p§]Øõch?e"`úEF?p§]Øõch?ïá/Zê?o»òµð·k?nФý3ʘ?o»òµð·k?ïûŽ@A…ÿ?0†–ág^?AÆÿ
²'?0†–ág^?ïæÿ嗸³?n35Gn®P?iƒÄ-2?n35Gn®P?ï­³¡¤ø??‡¹ù}³H½?""§ïü/?‡¹ù}³H½?ï¿&Ù* ?$›[× ?€86<¦ô&?$›[× ?ïàKO¼ß?f8Ê*"ÖÍ?o´rÉP'?f8Ê*"ÖÍAGN4FGL J2353.7-3037?µ‰^ÀS9Ϫ͞"À:7\óöÝBÀ<}:Y˜!Ê@ÇO"L«T@©3]$žE?¿¬Ð6f?¶a·U\ä?ö,û
͹\@¤Žèe¯‡?ï¦Á4éÙ¿ä?£ƒþ'¿Þx¹d»•¿à¡åÎ%'a¿êºM8—÷¿á4ÂkñAGNbll3FGL J2353.6-3037PKS 2351-309?ïÞäï?kUÊ#²‡0?pö
ïT?kUÊ#²‡0?ïܾ\'É?ˆV\.ßNu?qþ ½ ó›?ˆV\.ßNu?ïŸ+çpÌ?"ê[)ѝˆ?ˆ5´1?"ê[)ѝˆ?ï«rèˆr³?p2ܓĹr?…#EӔ8?p2ܓĹr?ï*½Ûd·‡?'˜Qö?š¨D"i?'˜Qö?ïZ?üfºÁ?¤WHD/?"¸v˜CË?¤WHD/?ïFO3;c?'5¹"àz‹?—<– w˒?'5¹"àz‹?îÛí%Î?Žñq­þf´?¢A/EÕ ?Žñq­þf´AGN4FGL J2353.8-3911?¼#0‹¬'ÀR?Až0PÀ;	æ~OÀ<Á|Ôfõ@ …±…@ïó»NH?ÑbäRzv?ÅVV"÷Q?óœ}YÇò@Æí­B?íü݀ú}¿é$â7˜¿ä=а‡é¿å^à
AL¿è5é
†¦¿ïÿþBe«+AGNbcu3FGL J2353.7-3911NVSS J235342-391442?ïúXqí>n?G¤˜ÌëG?Fž7øªJ?G¤˜ÌëG?ïò§"ª`"?Y¨éC'('?Z±º£¬í?Y¨éC'('?ïÀSØ¢Ì|?€RBá?Öž¢1?€RBá?ïóƒ»i??°{š?XøŠe«Ò??°{š?ïé	¬¯©"?hð˜'Wt?föS ;ôH?hð˜'Wt?ïÌðO)?€ºº™?y‡ØW>³?€ºº™?ïJ°Iðu?')ÅЅk?–¿‰õ
#]?')ÅЅk?ïÆRûœæ?j?‹˜~?|øVœN"µ?j?‹˜~AGN4FGL J2354.1+2720?æèé#ÎÀ@çu¸eÀ:ÖƞµbMÀ<›
ü³Df@x>He"@Òµþ,Á?ːßò?À)á¹mõ?ô}_Üßiˆ?ù§õ
j¿Ü°h}—ÛS¿á»'Á^Á¿æÒ<çè¿Æ6`y½[@¿îƒÏBrì1¿ïÿî' ÇAGNbll3FGL J2354.0+2722NVSS J235402+272328?ï÷xa]	"?GöQ »?Q=¾ßÈ?GöQ »?ïÐÁ/y"?{:ô*.[Ä?wŸh-@v?{:ô*.[Ä?輦ˆL•/?N§‰Õa?†YÝâ‹àO?N§‰Õa?ïŠc$Xt?qԄx^"D?g6Õ[?qԄx^"D?ïóь,Ò$?U•W¿&j|?X\çtáXì?U•W¿&j|?ïLՐb/Â?œ½Íøé?–eM¼?œ½Íøé?ï±uGWÐ?ƒsfåt[ð?ƒ¢›ßcº$?ƒsfåt[ð?íL\ÉsjË?£zvì*?µ²¬Û®?£zvì*AGN4FGL J2354.1-0958?sÊyÀQ
Ÿ¸fäÀ; ïܸÓÀ<|ùûA@ŸXŽâ[@²c"úÎ?Ða؂b›V?¼_õÞéÛ?íï8œÿ¨@Ý›ëÙW?î®X£/D'¿èÍ_ߎ›d¿æÆuÐfµA¿ØxÕÔ³K¿ë{¢´¿ïþaå£2AGNfsrqPMN J2354-0957?ïûÄ<cN?2»0~?@ïH€/ ?2»0~?ïì?¬›Ýt?gnWxñ?cÀS'Ý;}?gnWxñ?ï䬐Ó]œ?mšá¹Š"?kSo^Ãî?mšá¹Š"?ïñ«ñWh?Cu"ÔY˱?\¨	·ú?Cu"ÔY˱?ïü›PþÃ?4՛%P:?;'¼¿†š?4՛%P:?朗Æ@\?Œ'­4:¡?†ÕŽlˆÍ?Œ'­4:¡?ïê¼,Ò­?p»ÆçóÖ9?eCÓ4›V?p»ÆçóÖ9?﯍çL#?s‡ýNš£Í?"†2†}o?s‡ýNš£ÍAGN4FGL J2354.6+4554?í¬l52gÀ/¬ÚQÎÀ:¤l™†NcÀ<pÈÜ}Cø@2êm·A@=Û?VW?È)Eßaô?Òð ÿê[@1o† ˜'?îo\k«¿íh­aÍz?ïÔÊ\°?¿åã$\֚¬¿çèŸ8iÿ¿àoUB§šc¿ïþÍ?äF'AGNfsrq3FGL J2354.1+46054C +45.51?ïÄ¿sY$E?›ýõ`U/{?} FVÝyœ?›ýõ`U/{?耶-prü?È|ó.f?Íý'J>4?È|ó.f?î–hØí¨¡?™Ú­jnÏ?¦™rq%uõ?™Ú­jnÏ?êÓ¡t¦½f?§E	{R'?ız-e
h?§E	{R'?ï¦.'«¹?"–d¹p­?†t{'–¡à?"–d¹p­?ʙ¯Åf7S?Ê2óó,]?éY"¦r+?Ê2óó,]?ì¢"ª­pÅ?¨?,‹*±?ºîꪔyÛ?¨?,‹*±?Ñá¸à9n¿?·º'µF
?ç#ãH ?·º'µF
MIXED4FGL J2354.9+8151?½0‹k·@39¸ºÇËÀ:*Ô2ò›"À<B€'،@D5݇…@ÝÊeê?¤?À.I¼ât?¶y<×Ì°?òF>¢‹±@®õt‹Ã¿Ð-lŸ»q±¿æHdˆ?Õ¿æ=ò^¬³¨¿è–6—k¿ëpù'7}E¿¸—ß/OúAGNfsrq3FGL J2355.5+8154S5 2353+81?ïø#,!h}?G<SBr@d?OsO€;?G<SBr@d?ïï<§ìL?aÑÆK?`ÃXäV"?aÑÆK?ïãj%Á8M?kðKÅV†?l•Ú:¨+[?kðKÅV†?ïÙR™Ld)?X¶YöYL?sV³K_‰?X¶YöYL?ïݾ5œ±?ló@O,	?q ånRoÄ?ló@O,	?ï±'a»(W?ˆŒlh¾?ƒ¶''ÇŽS?ˆŒlh¾?ï¼vb:?…v¦d()²?€úâX«
?…v¦d()²?îèŠ<Vl?Œ‰tÍ H?¡w\?âg@?Œ‰tÍ HAGN4FGL J2355.7-3351?ï3¤Ý
ÀSzž+ϒÀ:,ÊëK=À<™QþÐU@wnåhz@€öÍ0 ?µŸÍ»4I?Ÿ¼*¤T™Æ?ãa¬ÃB	@õÕt'!{¿Åì]÷,è¿æ*—MŽÿ¿æq?2oê¿çäû¨'k¿å#'@ßÄ ¿ïéþ¡[.ûAGNbcuNVSS J235538-335225?ïü¥—{Ã?J¹—Sïm?:×ˎüÊ?J¹—Sïm?ïæQž_?s'ï!•ç?i®aüA(?s'ï!•ç?ï³s"1•?…NàmÓ?ƒ#"«?…NàmÓ?ïú¹8_0×?4{ºrISÒ?E…Ì©N?4{ºrISÒ?ïýY'°Òy??Íò¤È³?53è{?Õ'??Íò¤È³?ïkM;?žæ0çw ?'Ÿž" Î|?žæ0çw ?ïœl²°ÁÔ?‹¼z­
Þ­?ˆäÓ^^ß?‹¼z­
Þ­?ïíÎFkí?TÞ•Î,?bñ1´³ƒ?TÞ•Î,AGN4FGL J2356.2+4036?Ìd]f|PÀ52¹¯æÀ:"ØÛÎÈPÀ<Z¾ÎÝHE@ =û¹tUg?þْx=(?·0t¼ëXS?ª\Šo…?ՆŸ Âg@ͅþ‡/	¿ï¡ºÃ.¾?ÿ (¿ã'! 
ҿٛÈ]|\ó¿â"c'0qb¿×ïHÂçp½AGNbll3FGL J2356.0+4037NVSS J235612+403648?ïýpÉkÄI?%niêŒ?4yµ@2^?%niêŒ?ïó6sãO?^<+¤Óo?Y"<·a?^<+¤Óo?ïî{;h>‹?`Q°+>bµ?a"Äg¦ìä?`Q°+>bµ?ïà&Ô*9:?X8¡Ê|"Ù?oÙ+§¹?X8¡Ê|"Ù?ïú.õ‹ÝÄ?=®WgÐb?GD*ÝêM‡?=®WgÐb?ïÅËÐb??"4'€¾$í?}tˆ¬±?"4'€¾$í?ïí•)rj+?l—	¯FÎ?bjÖHÝ¥ž?l—	¯FÎ?ï—&8³j?|u1ÚìhÕ?Š6$µ®?|u1ÚìhÕAGN4FGL J2357.0-4840?Ìó©)ttÀP:ÎÄÀ:ꋨ?OÀ<È«Yµ}ü@—Ì±Éç?ÿ¸j1Í?ÅÑH#w)?ÁèN2'úC?ûq¹_ã•?úý¿é+ÿbKO¿ÝŸæ+]Ò¿ãµ…Q8¿ã"ñ10#´¿ÚNÖ½;ŠE¿ïÿÚ
¢ñ1AGNbcuPKS 2354-489?ïüUâpß?EÃTÖ-<??R½ñ<?EÃTÖ-<?ïè<ôõWR?réO/Ú5†?gÃ>â½Ê?réO/Ú5†?ïÌ2bþ§æ?~›ÖÂe[ø?yæΕù Æ?~›ÖÂe[ø?ïì=u¬T‡?KOËÙ?cŠbÉÀª?KOËÙ?ïï
•7è­?`©¦Ñ_a?`õjí3œ?`©¦Ñ_a?žeõí?–ˆÐ"Îl›?ŠY˜w°¬?–ˆÐ"Îl›?ï±±øZ«?ƒIÉ¢ ÔK?ƒ"¹¶ê•9?ƒIÉ¢ ÔK?ï_;;>è?…¢zO¾»?"žŸwZÿ?…¢zO¾»AGN4FGL J2357.4-0152?è|p+¿ªÀNÏÝ~Ë·úÀ:z–ê'°qÀ<zô/è%@LN†öª@ñ*_Oð?ʪ¾ZO?´‹õÈ|Ü?ñ"4 ½@;ª%-?½¤Òݲù¿å_×5ÜZß¿àHBY@ãö¿è6±•+v¿è‹D× ef¿ïî¤"‰—ÄAGNbll3FGL J2357.3-0150PKS 2354-021?ïùüµÂU?P9¼X?H܂c4þ?P9¼X?ïïSyÇ
½?bQ61ÐB?`¬†F°²s?bQ61ÐB?ïâêÕî«ç?v!Ä­ç×Ý?m)Þyá+?v!Ä­ç×Ý?ïö08W	|?;õ›
،3?SŸÈ—?;õ›
،3?ï÷Ålcß?Ra´ԃ?Pu'¨õ.ü?Ra´ԃ?ïµeRê¢?Ž¯_k?'¦Ÿ©‰i?Ž¯_k?ïÈÎÑðß7?'Ÿ›#üñB?{˜—¾pq?'Ÿ›#üñB?ïßt¨¯M?]Gzͯ€v?pE«¦!•d?]Gzͯ€vAGN4FGL J2357.4-1718?ç—%屎óÀRˆÂß
A1À:;<ó¦UÀ<C³aÁ»ø@ ãÍJ 4©?úü´=Š?¿ÜhKBôq?©÷#́?îmÓ­'ž#?ù ¤äüD?ïÝÍ:°Õö¿ë>³>±@ª¿Ø}[À›<¿Åó.ö¸ƒ•¿Ýþ‰Þ:³Z¿Ö›V½ÑÝ-AGNbll3FGL J2357.4-1716RBS 2066?ïüJ9Úu?2¾ÀåV?=¯QÉB
?2¾ÀåV?ïåëÒÕ.?lV¨Þ§?j-B[)Ô?lV¨Þ§?ïïFâg"¸?XûÊe9á?`¹˜lGý?XûÊe9á?ïÈ©‰ü˜—?csÛ	B?{«:èF˜p?csÛ	B?ïõä.yvJ?NoH-ç.Ù?T7£\Ê\?NoH-ç.Ù?ï€4Üç³>?"¤ËӇä×?òÈÓÑ ]?"¤ËӇä×?ïê4N'2˜?sXãxö?e˱tLÈ!?sXãxö?ïH¶áÇs?"®çŽ¸ø¬?–é#æ&I?"®çŽ¸ø¬AGN4FGL J2357.8-5311?îþ8
á¨ÀO
LÂPrÀ9³v/1EóÀ<B­Vœ@œÂ†!í'@…	¿œ?°1¶±W{g?"°Y_ÓáO?ߨ8ã÷5×@¨(#µ'È¿ÔDx $ο槹ž¿çK|€.8£¿æšD¿ë^œ£9UŒ¿ïÿëJwAGNfsrq3FGL J2357.8-5310PKS 2355-534?ïý¶Iܯ?'ýoö‹ñá?2M²òMhR?'ýoö‹ñá?ï÷WœÁc¯?QIF®"Ê?QPÆE!°?QIF®"Ê?ï×y¿'?xgähfp?tCz'¾@?xgähfp?ïÿìÑ=ä>ØÍ
œö6>ã.†¸ô)>ØÍ
œö6?ïþ¿ÈQ?ëMF?$€{°‹?ëMF?ïߏG¸É?r!T¥8©?p8xê'÷–?r!T¥8©?ïØDSŸ˜?y²ÿH€?s÷]̑L?y²ÿH€?ïÿàݝKø>êTN™¼Ü°>ï"DIº°>êTN™¼Ü°AGN4FGL J2358.0-4601¿×f%õn<ÛÀQÇ%ÃßÀ:UŽ7£À<›£í°r#@üaŽQ@Õ8ü Ïï?¶Ml€—ü¿ !`!þ­p?ä)šÞh*·@f÷1OXX¿Ý§dŽu¿ä³[wN¿êeøí½]¿â¨¯à-¿áîKØE¦Ó¿ïÿ¢­>'AGNbcu3FGL J2358.0-4552PKS 2355-461?ïþŒ¸éÄ?~os‰?'4rCó¾?~os‰?ïöy ¨A'?T!t'£¯?S
¿q0î?T!t'£¯?ïêó¨P¹?g…'Tɬ?eoOp7?g…'Tɬ?ïÿ•	oû>÷KÀÏGà±?
½šÁƒ±>÷KÀÏGà±?ïþx¡ý@?(('#‡Œ•?.hwiÌÙ?(('#‡Œ•?ïÙbI¡3Â?骭ae?sNÛXÛ:?骭ae?ïàM¤'_Ø?u5¸QHO®?o²[ªGe?u5¸QHO®?ïþ½æÄ´?$§+½"*?.ĸ·ˆÌ?$§+½"*AGN4FGL J2358.1-2853¿èpš}!òLÀS‡óõ"À:dü'¶vIÀ<œBÇû¬´@ŸpÕ*>m@ žÛøº?Àv†š
‡Ó?Âø » ýÑ@}¡›Æš"?þYÖ)ÂÇ?؉хCKY?ꫦ!r™¿ç49ÀGƒ¿ÛÎó£PQ§¿ïÿ½_œr½?è[¨«AGNbcu3FGL J2358.3-2853PMN J2358-2853?ïՇLÿ¦Ù?rêçè[I?u<YlîÃÕ?rêçè[I?ïXf|œïÌ?¨ÊH8("?"ó0jª8?¨ÊH8("?îû÷_?"ÚÇ»™˜? OHŽŠ?"ÚÇ»™˜?ïyÕâ}Â?‡iåíÏ	?ÐÅ>ˆÝÒ?‡iåíÏ	?íT£Mw'?´Ûgÿð?µZå'úÅ?´Ûgÿð?êW³ë í-?Í´äù"V?Æ¡0S|KL?Í´äù"V?î}nY"?¡7LBYß?¯Nh)öMÄ?¡7LBYß?êsiµŒzˆ?¶À€ÔŸÖª?Æ2Y)ÎÞ?¶À€ÔŸÖªAGN4FGL J2358.3-1021¿Úƒd'`±ÀQE/Ÿ¾wÀ9Q}˜²
À<,ÄFŽ@jÉۀĶ@å:Ü?¯ÁðOÞº‹?µ\â?`ú'?þž"_¦XÅ@­Ô3É[(¿×Ų'¸#È¿ãðÝî]@M¿éR0^—ÿ¿ç2çHy–¿ìd¾ÆyÌ¿ÚäVÁ­´ÚAGNfsrq3FGL J2358.2-1022PKS 2355-106?ïþ6u²à?#.Òêü,¹?/¬™ûÞ8J?#.Òêü,¹?ïïÚwœ[?cfª¢E²?`%ˆØ…­s?cfª¢E²?ïççéÄæ`?`	@¬©§ë?hF`E?`	@¬©§ë?ïþçù<Ü?~ì)~Ž:?!€h3²ÂZ?~ì)~Ž:?ïþ=uVnL?%Íæ/Mæ?,(«ÿŒ'?%Íæ/Mæ?ï¯K‰/-?Ž°råT÷â?"-·Le:?Ž°råT÷â?ïØ;çülç?vÜoW}Í?sâýª_?vÜoW}Í?ïüƔúMŽ?1^T4Ij2?9ËX}Ò¤?1^T4Ij2AGN4FGL J2358.3+3830?ÁH>)¨½EÀ72"áÉ´À: ôX,À<HÜ}Cø}@®Ö€Õ¨i@R:¸b²?»hŠØáƒ?'-c÷‡qµ?ÅŒ:
'Ö@
™dôÌE=?ïd' ÷¿ÙLo"È&J¿æ#׶ÿ†¿á'‡N={¿ÛMh=¬¿ê#¹B¬LûAGNbll3FGL J2358.5+3827B3 2355+382?ïþ'l	Ϟ?"t†z¾?&é=}
2ä?"t†z¾?ïôy®J?`Þj±]0a?WÜåd[O?`Þj±]0a?ïø"«£Ì?UïûN`?M¯Î*aÁ?UïûN`?ïüÚvƒ"õ?#]ñ¦Áj4?9,LÑðfh?#]ñ¦Áj4?ïþ!ù"?"YEO[ž'?/ÞÜ`42?"YEO[ž'?ïÊg·hÑ?†a‰ù6º?zÌ}#›«b?†a‰ù6º?ï÷ɊÍùÉ?e·6q"?Plê¦îž?e·6q"?ïùÐúž?8ù.©
U™?K¹‰°,û#?8ù.©
U™AGN4FGL J2358.5-1808¿ê¿ï]ŠÀR·D»ó¡À9Ø<Ç0«™À<<4ÿ¼
b@mS[?ýЋö–Ë?¸Š×´ÝAå?«à©^Ä£?õy²X­@@@tÁï•?ïä‹?Ž¶<?ÁK°B'—Ê¿àÞ¬É!F¢¿ÕçÓäC6¿ßMJ 4¨Ô¿åÎAvÂÔüAGNbll3FGL J2358.6-18091RXS J235836.3-180701?ïþV8µ—ì?!ŸBÿ½àÐ?*œvoæÛé?!ŸBÿ½àÐ?ïëÔÜ)¥Û?s͋0æ?d+#õöK?s͋0æ?ïôz¬!9>?]ÊcCLØ	?W
§ìH3:?]ÊcCLØ	?ïï¬t"øº?J"4+)<p?`S‹æ¦.R?J"4+)<p?ïûÞ+U)Ž?7w9ÐX@?@‡Q¬ÐQ§?7w9ÐX@?ï¡{­ËTÓ?…c¼ó¸?‡¡*Ë[?…c¼ó¸?ïñåýd3?lÌEû!Gó?\4ŒÐ4?lÌEû!Gó?ïܬ"P¸?bLª¼ÐU?q©µ»w0¬?bLª¼ÐUAGN4FGL J2359.0+3922?ÝeôC¼ËÖÀ6cÓ^·E|À:bylÓgòÀ<7g0Â@Â	O_@é~¿\¢?¿y$?`¤A¿'Å˞?ÑB>éÊ´@
M|'¹Ø¿âïãÂwß¿çѓÛêw¿âÄ´š¦ßÓ¿æ*Ac¿Þï2²¾.¿ðAGNfsrq3FGL J2358.9+3926B2 2356+39?ïþø[Š¯?#"ð€!ßD?/|$…32?#"ð€!ßD?ïõOë"[?YÄp2œ"I?UaøuΊ{?YÄp2œ"I?ïðE»~¤S?fboÿžÞ‹?_tˆÀ¾Ù"?fboÿžÞ‹?ïÿ؍uI?ûTîG?ñ8?ûTîG?ïü/rM>;?8@ Pß=?>"o'¢ñŠ?8@ Pß=?ïюó£PR?ƒ¤"ßib?w8†IÔ·?ƒ¤"ßib?ïì9yžQ?o'b™µž?cƆ9Òøù?o'b™µž?ïüøµ¡?- Áoԙ!?8?Ó/ôO?- Áoԙ!AGN4FGL J2359.0-3038?ïÖ¨©éÀSŒSâÖÀ9ô·ˆ—é–À<;'&¶M/@ o"üT?üÈÄ3¡?´ ëóX§·?'«¥''"v?ßµ<ã5D@œåT-)?ïþé+0/¿ã'[ßú¦û¿Üôú¸îI¿Ô="_ÑKã¿ßQÞú¡Ç;¿Ó·'¸¬"XAGNbll3FGL J2359.3-3038H 2356-309?ïûÊü	°?:Íé×Î?@Ôož•¾?:Íé×Î?ïêÃmÓm?nujšèv?eø<TS›1?nujšèv?ïÔ¥+ѝ ?{¨I®z	?u­jB4A?{¨I®z	?ïðèü¿iô?J;	Á[ye?^.Î#Wª?J;	Á[ye?ï÷ó¢W5ú?L6¤EW?P»ÖÇ>?L6¤EW?ï–NÐ=?")k_ÿ¬ä?Šl~~A@À?")k_ÿ¬ä?ïÆÊjO‡°?"­¼…9·È?|šÊ¹O¬?"­¼…9·È?ïá‰4œ"Ì?^iAÁý*?nvË>OlŠ?^iAÁý*AGN4FGL J2359.1+1719?ÑR#¬`#_ÀEâà"&þÀ;5áAÎ×iÀ<µÿÚ$@À€ŠÔÚ¸?þfv÷®!ç?Ë©…ïm·?ÅGФÕN?úÀâ³¾ß@¾ivf9¿ë‰¤>8Ió?ïìl5ç¿Ë7dpB¿å^"ñ¿×h@zi¿åƝ]É^ÙAGNbcuNVSS J235901+171926?ïþlR[?"ñKfu|¤?/‰7_´cÔ?"ñKfu|¤?ïèÒ.M?kM딼Ò?g-Ò.:·?kM딼Ò?ïۊ" /­?rRyî
ç?r:½È¥YA?rRyî
ç?ïêg–
H?MŸ
ŸÓ³Þ?e˜€DÖð!?MŸ
ŸÓ³Þ?ïùcwYäß?FFÐ`g?Jr"":¡?FFÐ`g?ï¢ÈŸk•¥?'{<î:3A?‡MØ˽?'{<î:3A?辶O"Õ?†k;›Dø?…–l©fÖ?†k;›Dø?ïšFÎN4Ê?zkX•LÀ¾?‰nLsR|?zkX•LÀ¾AGN4FGL J2359.2-3134¿àîė°F•ÀSsC¬ÄðÀ:Ê§XžþÀ<Œ5¶›2 @üЁ¸&x@¯¿%D]'?¾šòŠ ªÅ?£ÿk@Ñè|?â%Ûüëx‰@ÌÆ+$q¿±=´€û"	¿ãB©D1ˆ¿ê-b
ç¿æAµaÌ"Ù¿éKŸÀûs¿ïü{Eñ{ÙAGNfsrqPKS 2357-318?ïҘr?¯Ê¾ÑGÁò?v³ôÔÑj?¯Ê¾ÑGÁò?ïêÛU¦¥œ?s~·¬bÅ?e$ªp·¼/?s~·¬bÅ?ïÄé7?|ëíD؟X?}‹rw´G?|ëíD؟X?ïÿ'_…Ãñ>ü`ÓÆÑ8?¨ÆÌíÒ>ü`ÓÆÑ8?ïù»lA
¦?HVÛc¨mà?IOÔ'±?HVÛc¨mà?ï›h|HÙk?uËí_Ý?‰%àíÉ¥.?uËí_Ý?ï¾×ž.v,?€€_JŽ$¹?€JfLõ?€€_JŽ$¹?ïþÑOχM?ž"'Cùü?"ëO2³‡?ž"'CùüAGN4FGL J2359.3+0215¿íóâ¯{ÈÀM<ÿdύÀ;b:	ç
À<´a‹·@ ëþ±Ì@`?ù·ãÑÌ?Ó˛ÿûMi?Û—ßÛq@ó‡œAÇ@ÏÅwÃÜ?ïÝH°rùó¿ïÿóÀ¬ƒ?ïÿ¤Á	¿×¾?kOÚ3¿àÞ¾fØ|¿æzD5ëAGNbcu1RXS J235916.9+021505?ïüOÖ5=?4Ix²>·?="½3iN?4Ix²>·?ïæ%ëÄV(?o&LqP?iÚ°*?o&LqP?ïÇÖ@Çy?sŒ‰5>j?|ß³ Ö ?sŒ‰5>j?ï¿Þá2›š?jZÊÛiË[?€G¥òŸ›?jZÊÛiË[?ïü*Õ/‹£?;þ«y~×?>©X@ðHp?;þ«y~×?ï"AÃÄ»[?"§ßx8/x?‹/™?"§ßx8/x?ïÑ|þòþ?{·99Gú_?wA€"D¦?{·99Gú_?ïi·•>Q[?ˆ°¬øÊkC?'É
[¥p§?ˆ°¬øÊkCAGN4FGL J2359.3-2049?ž¹
=¿«ÀS"¾7ޓŸÀ:Z€U$õƒÀ<‹³¢,@U¼!É(@øУñâ0?·ç
¶<h¿›€ØúÏáÍ?ä6wÁ½o@8¶Ñ"¿Û¯©ü=RÇ¿æ‰RÄÈòM¿âR°Ü¬=á¿Ý¡z¹"œ¿Üß!c'Å¿ÞÎÙAzHÆAGNbll3FGL J2359.5-2052TXS 2356-210?ïøÿQåÑ?Bν.Ëw¿?L•Ç·•?Bν.Ëw¿?ïï"_)‹?c
ÛHÝ1Ó?`l ÍJ ?c
ÛHÝ1Ó?ïïSþ§2?iŠLi£ÿA?`ø«ÀÀ&…?iŠLi£ÿA?ïúá#,;.?.k°:5?D{rs¹Â?.k°:5?ïઃ¤ ?l™ƒZ…?oUýI¨0?l™ƒZ…?ï¨<]Ïá?îwÂYV^?…ðÿ6Jwš?îwÂYV^?ïçcnTÇ?urî%_O?hœ'F?urî%_O?ïê³ ?V¬sˆXx?eL_ÕT½?V¬sˆXxAGN4FGL J2359.9-3736?ïàËsöÀRºÛŸ'xÀ:òêÏS)À<ËR—|ˆè@8¦ÿ´?þ'5deÛ&?ÇrÀF׀?Т‰bñO@Ô×ãD8?ÿ‹O™Æ:7?ßð̆Uï÷?í\૦âW¿ÚdéÄTXG¿àJãq*¿éÓYG™ó¿×¸4½¤¼AGNbcu3FGL J0000.2-3738NVSS J000008-373819?ï¬å°bLÀ?'åSnv‡?"Æ"Ù®`?'åSnv‡?ï¶Æü ?'ÞC‹¨¼¹?'x?N˜î?'ÞC‹¨¼¹?ïUŽJc¯?ŠÐ©>ã?•N6ºiWc?ŠÐ©>ã?ï'Xdg€?rOò²•¹?‹©æ鏘g?rOò²•¹?îª~ˆ
ï?¦NN%Ÿù?¥X}¦ó?¦NN%Ÿù?îÆfF£l?¯æ–XŽºØ?£™–ù??¯æ–XŽºØ?쑡€ÌKÑ?¦¼áª ò¶?»róù¡w?¦¼áª ò¶?íÛN;¼œ?œ}Q¤gÆ?±%Ž!CÜ?œ}Q¤gÆAGN4FGL J0002.8+6217¿ÞÒ¼ó2_¿ª!gâE­À8Áœ©'žÀ;^`¯m@u@Ý®Éü¹@‰øÜö¼?®'‹`òË?Übþ<†n@%C1T??ü±åÃhÊð?Áºg"ôq¿Æ|Í[g¿á©c;8»¿çBëØ*Îá¿ïFMä¬g¿ïÿÌ~sM€PSRPSR3FGL J0002.6+6218PSR J0002+6216?B{rAÕ??c¬x=Ôo?ïûaMçƒ??c¬x=Ôo?²æ`¯?²¯(ÇÖ`"?í®PÚ*?²¯(ÇÖ`"?"þH†1?{t
UþÁ?ïgçÇò>ï?{t
UþÁ?pÏGDÇä?aJç?ïÞaqnø?aJç?CºÌFKˆ$?0£²@ìCµ?ïûLó<'?0£²@ìCµ?ƒÊ,öa}j?‡}À'Öf\?ï°×L=×b?‡}À'Öf\?ƒä¸Êac?fË;È%z?ï°m½aŽª?fË;È%z>ù甑0ü>ñzJZÓáD?ïÿÌ0š§Œ>ñzJZÓáDPSR4FGL J0007.0+7303?î¼,wh}~@$ìaR*o?À5'c;8»2À:xM'Ðÿa@.!|Òc?ý¯Qvëè?€"'—s¤'?ÑøÁ²½W@QTeâXO?ú$¸÷WåÅ¿ I[=¾QŠ¿É)ùù€´ñ¿Øör¸"@l¿àÏ>šõ9¿êˆ6šÆÀC¿î³'#iPSRPSR3FGL J0007.0+7302PSR J0007+7303?v,î(œÁ>?z;7nCd?ïÓ¦#{ìF?z;7nCd?'/ÌþI.?•–ï£ÄôD?ïn˜Fv?•–ï£ÄôD?¾¥¾"ÏKò?¬±<ْ<Š?ì+H/f'?¬±<ْ<Š<YR$Ê>œ<Àç7?Ήˆ?ð<Áº	*ïÇ?gHÑ°tò?\h<oö}?ïè·äTË+?\h<oö}?fêŨ?snUÌyç?ïéáF_?snUÌyç?ž|ÃWՕM?žS¶£zþ?ïåjŽ¥?žS¶£zþ?ðPSR4FGL J0023.4+0920¿»,'È~	ÀJrÁÁÖυÀ9›íQx™À<0j÷ŞÛ@…K2Åz?þ+O¤ƒ¨?¼J/¼P?ݞ7@.@¼æ")Æ@½f'|F¿æ‡Y%5C¯¿»,y@ïņ¿Ý‹ßœ³)Ž¿èqÊÛ[¿ëbœ!´/È¿ïû¾½?'PSRPSR3FGL J0023.4+0923PSR J0023+0923?¼M©¾C·?ÁªiºG©?ìv\ªÈ7‰?ÁªiºG©?Ѭ–=?Ŷ~õ±ûï?ç})ž´át?Ŷ~õ±ûï?ÎÛ̾xåß?³94û-Š?èIÐaƈ?³94û-Š?՝4ÿ;4	?¶!ªdÎþÚ?å1e€beü?¶!ªdÎþÚ?zèùnb?}u	úý"/?ïËø.$€"?}u	úý"/?°t†?¶<î²u•?íþþ1b'`?¶<î²u•?›9Sê«•?'Òµ&å]m?ï&5`lt?'Òµ&å]m?"bVøgI?†Ô	îEŒ_?ï\íHdÀ?†Ô	îEŒ_PSR4FGL J0030.4+0451?ïú{¹YåÀLÎi­BÃÊÀ7‹…º¿"À;‡^@'7|@Vÿë]0³?ü"µ—&"?š¶‡øºm?ÜzRõñ@?þº{'pÖ@¸wù
îF¿­@}Ú²z¿»Æ¤i¬A¿ÛŸv¼Ï)¿çŠ©Üݼ¿ît‰u_(¿ïþQ>¶ôôPSRPSR3FGL J0030.4+0451PSR J0030+0451?|Ft{K~š?‹•LZò¹?ïÇs֎Ë?‹•LZò¹?¾ÃÓe(‰ó?½z°92"?ì'…"ZîÂ?½z°92"? (}J*d?—\þ³¤²§?îýx+4â
?—\þ³¤²§>t»€"'Œ>†û|h(H"?ïÿÿ×¼>†û|h(H"?€0ÌÀQX?¡!¢Ärö?ᅮ<Ìþ»?¡!¢Ärö?š		÷¢#Ü?Ÿ›•¸²@?ï/·°'r?Ÿ›•¸²@?æX3ÿ©?"PŸ&	Í´?ïˆfžùœ?"PŸ&	Í´=ŠL6Å
ç=¾ã¶ø¾ë?ð=¾ã¶ø¾ëPSR4FGL J0034.3-0534¿—b£®Þ^ÌÀQ³g ù	À8™¸Øú¹À<øä@bFg'A?ÿÕGª¹|Ž?¥=mbÈÂ?ÍیÙÝ@%Û°_®¼A?ûåÛÏI(é?¤7ÈÄ)¿Ô5Ñ>B¿áõ6þ™Îs¿æ^92¿í=¶y¤0Ì¿ïþ×@ÄnPSRPSR3FGL J0034.3-0534PSR J0034-0534?‡ðcý@ã?ˆc§¢ÏUò?ï >pAö3?ˆc§¢ÏUò?Å*e¦šUy?À¥GíÕ[?êµf–Yj¢?À¥GíÕ[?Ñú¿}©b?±b¥¶ý:z?ç A1+O?±b¥¶ý:z?™[©ÍXà?2*m¾~¾?ï5"±°¼¡?2*m¾~¾?v†J@šÁ¹?qÀ·RU¥?ïÒókXNÝ?qÀ·RU¥?§°^|7?«pz2z@?î"úh	\?«pz2z@?Å=F»þk?°²E5Ìè?ê°®Q?@e?°²E5Ìè?6Å$ò©Ô"?3͛Õ-n›?ïý'[l?ø?3͛Õ-n›PSR4FGL J0101.1-6422?ímU&‰<æÀJ]c
'SÀ9nŸÀ<]
þÆD@3q¾‰=?ýút?¬î ‡—Æ?ÙÁ9d@+ß /µÐ1?ýMÌôåŗ?ïçlá)Ñ
¿Ï5¤&»V¿Ûò ›ìZ1¿ç"ò5<!ï¿ì«IúõÕ¿ïþó%&*6PSRPSR3FGL J0101.0-6422PSR J0101-6422?zw;í_H? –Mß?ïˈ…€? –Mß?ÊòOÆÅTf?ÅE7nΌ7?éClNªæ?ÅE7nΌ7?²?4<Um[? äÏkñ<?í¸xÏ4? äÏkñ<?t:5v%–~?n`›˜AÀÃ?ï׋"ôk?n`›˜AÀÃ?kT2#—Ž?k‡ÆUŠÜ?ïä«ÍñŠ?k‡ÆUŠÜ?°b¯ñ¡x?¯LÅúw_E?íþ"©ô
a?¯LÅúw_E?Ÿ<ýËî©?"¹f¼Ã,u?ï¼ƒ?"¹f¼Ã,u?)è¾÷?	S͋?ïÿ»Xtúî?	S͋PSR4FGL J0102.8+4839?æ"U¢7½À,VÏ d#–À8ê0IsçXÀ;Óg'Æ~@Ý«PÑ(Ò@:Ì}?¬¼FÓà?Ðàâ"@"Ëê¡ô²?þ
þÙy•?ïƒÂwß5¿ÑØ)ø!¿ÝãJ<º¿âàe0¿ëÈ°ÞY½¿ïÿ¶Ï4†PSRPSR3FGL J0102.8+4840PSR J0102+4839?ƒÿ¼{Ugº?ˆ^'+
ÖË?ï°Ë)?ˆ^'+
ÖË?Ã|ÔEù?À®úBÀˆ¶?ë þ
?À®úBÀˆ¶?ÌCïìÀÙ?±†ÝÇk?èïÏü
?±†ÝÇk? >•'Óöš?Œè7Io?îü¦à?Œè7Io?j:Ñõޓ?_ÿqüMï?ïåÅ.üJq?_ÿqüMï?¤Ñ¾Ôm~?¨uä`-?î²ç#÷<H?¨uä`-?'4Þé`Õy?Œ(¯(b?ïvYëó?Œ(¯(b?FD›Ëqu*?<òƒ?ïúnÙQ•t?<òƒPSR4FGL J0106.4+4855?ïdöEZÀ+½í6´ÈÀ8©Œœ[úÀ;áiF·G@h'"ß-?ü#iüóÜ?ª]é?IA?Ýg.!üT$@/&VÍl.ý?ó½ÿšT‰?ê]»Çí¿¿EQîµ)î¿Õ™ –ö¿àçÉÉã¿î"Yáó¥¿ïþ¥AÃnÕPSRPSR3FGL J0106.5+4855PSR J0106+4855?TŸ×‹v?V©™7½:?ïõ°t?V©™7½:?µïî]ªÐÛ?·ÌÊ%V|?íB4sá4?·ÌÊ%V|?'•KM¨¡Â?ŒQ
h÷?ïsU¥NÂ?ŒQ
h÷?	FU¼N? Ò»cS?ïÿ·PÜ? Ò»cS?[P+¸7»?NZ¯s'™g?ïòWùï£D?NZ¯s'™g?•/é'N}"?›Gù}¾™?ïV€³LPÄ?›Gù}¾™?†]˜¬^ÿ?v§cÜF[?黎‰N"?v§cÜF[>™P'¬7q>¨bññËá?ïÿÿ5™ƒ¹>¨bññËáPSR4FGL J0205.7+6449?ÖCåCLl@¨Âa8ÿüÀ7n÷u³À;)®^L¼q@\íó@g™¼Õ?—Å
`¬?çQéßú@$wFˆz@ªIâøc¿­Èl뻥]¿à'5ÏŦ¿æ3ôÄb›¿èD¦ÃMÈ
¿ë~gä맃¿â²Áô+¶gPSRPSR3FGL J0205.5+6448PSR J0205+6449?ïHé 9"?¸ áXZð?ŸVâËø͘?¸ áXZð?»™:ä'v?»¤Lê®#?ìŒØ£o±>?»¤Lê®#?êõ·'žšØ?¯E5‰ç¯?Ä)!¹…"¡?¯E5‰ç¯?ÍÝZYN?²–èúª?舺©i¬?²–èúª?çNK)@†?Ç©=rô‹¥?Ñci­~äô?Ç©=rô‹¥? :V>ÛE?¢íni%n¶?ï~þ-f?¢íni%n¶?èxWôý8?¹4!®ß"¦?Π/œ?¹4!®ß"¦?s§Š#æ?dù 3Btß?ïرÀèú?dù 3BtßMIXED4FGL J0218.1+4232?ÒJ¼úº'À1"~"ÐÝÀ7Â>Nh‡À;aHt
@¿égã5@ô¸ÙÐÁN?Ø›À˜ê{?Çjþс½@)ÆP¤]B@á+'¿Ñÿ']<9¿ß-˜T<¿ä9‹!0Ò0¿çW_ã?€¿í$¯ÂzäM¿ïÿŸ‡ð#êPSRPSR3FGL J0218.1+4233PSR J0218+4232?Õ¬ƒ)`?ÏHɦj?åq)¾?kP?ÏHɦj?ÁôõF#áî?¿·­…"­ï?ë'®w…?¿·­…"­ï?áóÈÒÂ/?¶	05&þG?ÜþnZ{¢?¶	05&þG?'MXHL'-?"ÿù÷®?ïm•=ÙN?"ÿù÷®?ªZMSoê?®{uæ7â,?î_Ú[*É?®{uæ7â,?£
IW}c…?¤ÎDÝYÖÄ?îÏ[j^îx?¤ÎDÝYÖÄ?Øk^îLú/?»j:µ¢R•?ãÊPˆÙ'é?»j:µ¢R•?—j@ŽÿC?48tµÑ?ïÿDÆrY?48tµÑMIXED4FGL J0248.4+6021?ÏáÕZîk·?æ­Ü|m8èÀ8>°C)JÀ;
ïunA&@Íx¤¥Â@c]$žDú?°¯8½5Õû?áUÛ¿-ý¿@"ž9'û@¤»üoý"¿Ú\DNŽƒ¿Ú_
Q'™Ë¿â°£¡ZX;¿êuŒ\š5¿ð?ðPSRPSR3FGL J0248.5+6022PSR J0248+6021?ZûáØ5­T?iÙ'#.?ïò'Sù?iÙ'#.?µ£Aö›Î?³7H·AÝ?íK—ÝE¯¦?³7H·AÝ?¸IÉ»0©?¥ÆCPÁÛ?ìöÌG
R?¥ÆCPÁÛ?"íûŠi>Í?ˆò5ɱÖ?ï`#¬¶
?ˆò5ɱÖ?Ÿ›†ÏT ó?ÂÀÏϜÇ?ï#ɼT¸?ÂÀÏϜÇ?†i<¥9ð?"±Ý›À?鱗[(çø?"±Ý›À?ªf³EÁî?£|Î''à?îY"ÎP'?£|Î''à?"Ž±I?m1ÞL¼P?ïÿƒö¢½?m1ÞL¼PPSR4FGL J0248.6+4230?í«Ï}i–À.£^·E|À;nµÀ@ÍÀ=%(H¦@S9›W3î@‹o"Ný?̓ÞC¢|?薈¢ÑPÀ@ˆšˆ¬âL?õ7xŠ*eÚ¿ïÿþR€ÖT?ïÿÿ>¹ú¿Ù¨ ½Ð/®¿áó¢Ÿ&ÌH¿ïÿwy´!¿î(zÝì¯ÁPSRPSR3FGL J0248.5+4232PSR J0248+4230?Ö¦†&™?Î-ÔÜ]/þ?ä÷,¼÷l´?Î-ÔÜ]/þ?Õ´dD¼â8?Êɔ§Ø?å%ÍÝ¡Žä?Êɔ§Ø?àJ÷†E?³ §ï?ßÿjóuâ?³ §ï?À¨Z†¬Ø? R²ŒOq?ëÕé~^TÊ? R²ŒOq?Í-ùÔS-?ѕÆZɲ?贁Šë<5?ѕÆZɲ?µÚãè|"?¼þðý}'?í_£¹ê-?¼þðý}'?À´5Å<hD?¬<<¯#h?ëÒòŽ°åï?¬<<¯#h?€nʯWn?nôsuf¶"?ï½ÊD¡"?nôsuf¶"MIXED4FGL J0251.0+2605¿ïôÊùnÀ=~‹;26À:!["Ì´À<{¸;EPl@ÝgX(àõ?þ³°fd¸ç?×ɵÁ?äãkªs±@9à0Và@fw@(d"?íº@£^>z¿×÷½j.G¿Òn2b¨Á«¿æÜ>¯¾¿îú!~ÕÈõ¿ïû
ÝԇPSRPSR3FGL J0251.1+2603PSR J0251+26?´çý{•Ï?»]ô5Žq?ícPnÖ?»]ô5Žq?ÍÕ÷EÑ
?Æaˆ[-Î?节.»K½?Æaˆ[-Î?ųÓvà;?«ztF§'?ê""Gþq?«ztF§'?¿Mùj%€?¢ï::,"j?ì@Ò¿;P?¢ï::,"j?À5Zlíp?¶.¼¥!>?ï€ÿ*±É*?¶.¼¥!>?²eˆ(A¸h?µƒ÷µ/‹?í³Nû!C?µƒ÷µ/‹?¡;}{ù%?'¨¹ho?îìH(@nŽ?'¨¹ho?{"sö|ˆ?j|5K4ˆ}?ïÈ÷ˆÏ?j|5K4ˆ}PSR4FGL J0307.8+7443?ï3´.è˜@,p&grÕàÀ8Ûö"o³íÀ<Gö-fÿ@aßÀšdp@ã!ž¶9?§ãÐÊ][Ñ?ã¾]~
qô@1õÜy@àTÍâ?Ò®íÞë2i?Õgá:Âõ¿Ö"ÛÅc!¿æ_f¿ï¯âjmÝ¿ïÿÞ§À£ÊPSRPSR3FGL J0308.0+7442PSR J0307+7443?[Ù¿ãQó?[°^¬Y¡ô?ïòí[8?[°^¬Y¡ô?°­Õ~Y«?²£â'™»¢?íêE\ð4Ë?²£â'™»¢?£9
÷;?¯?–ñ綇Ï?îÌo cµ?–ñ綇Ï?5b ?•"?ïÿVTþè†?•"?QLêÝ,?D¨{>ôÚn?ï÷Y‹6ªa?D¨{>ôÚn?9<ša«ò?–÷nÔ!"u?ï~6uÁ?–÷nÔ!"u?‹3H³¡M?}xuS´s?ï'Ã2³ö+?}xuS´s>¤¹¼;¾©>'=Áµ%?ïÿÿ¹«B>'=Áµ%PSR4FGL J0312.1-0921¿ï®:6Ì^­ÀJ/]$žDúÀ9ù…¤ðñÀ<ýdDM@JXE;st?ýίá»v?¾¿<ÁQnˆ?ãª)Ÿ5ºÍ@!»/fÊ@>Ï5ݲx¿ïÿÿÊPË?ïÿÿÊPË¿×,åÜhKC¿æÊ{ÿÒs¿ï*Aò闿ïÿö$´ë/PSRpsr3FGL J0312.1-0921PSR J0312-09?›éÒÈ3Õ?«õþ¥[?ï ±o'ù±?«õþ¥[?Ïhpr¿÷8?Çä õݬ?è%ããP2?Çä õݬ?ÄæN2èà?°#2Z×M@?êÆlsEÇà?°#2Z×M@?À¤µ\ÿƅ?©œ6xF?ëÖÒ¨À_?©œ6xF?|0¡4L÷?¸`±èFÊ?ï'=¤j?¸`±èFÊ?µ
obÁôµ?»~€Ž…¿?í^²§Ái?»~€Ž…¿?¬˜k{Œü?¡ªbÈ)Øt?î6yHb¼°?¡ªbÈ)Øt?s÷¸ŠÞ"?i@Rá½_s?ïØŽÝAÔ?i@Rá½_sPSR4FGL J0318.2+0254¿éÂD6vð³ÀEË]9–ûÀ9ËɪiÀ<yÿ–M´¿@Ÿh#ÕÈ@lŸÞW8Ì?·Ô=À'o?â">¾°@ ã§Ú¤ý@–ÝàE{¿åC%ÿ˜üç¿Ç×±j¿×Ïxäl-¿äË»À5Ö¿ïÿúÁҝǿïÿÿ" 5•PSRPSR3FGL J0318.1+0252PSR J0318+0253?›3‹À	'G?¨ó5­Å?ï&c¡ºû>?¨ó5­Å?ÒjúÆko÷?ÈÅ©ºEƒ?æʂœÊH?ÈÅ©ºEƒ?¿û$ñHyŽ?§%*øE?ì›aÖðÎ?§%*øE?Êòö%Ðbó?©±˜½kü?éCBv‹çC?©±˜½kü?þmtEÎÌ?³þʘ6?ïˆJX$?³þʘ6?µz;Zt?¹j¹,}1?í]и"±}?¹j¹,}1?—TȐD^¾?ŠˆÓ¥cd?ïEY»T¡º?ŠˆÓ¥cd?'¡%Ä%¯u?qn©ä'ûÆ?ïµ{hðÉ?qn©ä'ûÆPSR4FGL J0340.3+4130¿ï¢`–SûÀ&%kÊSvÀ8ªµr£ŒÀ;ö5©/8Ó@šV=#vþ?ûVAU4æ?§ÿ	µáMã?Û¨Ÿ{°Ðm@/ŽŽ}Ü¥?øŠi
/®Ä?ï¶úÀoÇ?–ôu=å¿Ì?€Êë¡¿àÔÀŒ!·¿ëÙ-ފf¿ðPSRPSR3FGL J0340.3+4130PSR J0340+4130?d‹ÌH5Øc?gæìß%?ïët3ÈHH?gæìß%?µ5Kv?I?´›"óAx?íYV'ä'?´›"óAx?£ƒ#uûÚ¬?˜EØÚÕ¬£?îÇÍÈäú…?˜EØÚÕ¬£?,Æ `h%?*É`"Ý ?ïþ3•¿Ö€?*É`"Ý ?aqvÏ
•?c	—Ö8lì?ïMϟ?c	—Ö8lì?'ö\h5Éf?˜J¼Ó	ƶ?ïpM¾Qµ?˜J¼Ó	ƶ?†½­ùa¦?v
yb†1?ï¥	Gã¨?v
yb†1>¯1m6w>>¸æ
Ëz?ïÿþµÅõ>¸æ
ËzPSR4FGL J0357.8+3204?êYÿ>[¡À0{ÃŽÀ7qJEžpÀ;…¸èz0@Oð}+#ð?ÿÜЅ¾ñB?š"éß,Jâ?â{+ðHÒØ@B~ÉÀ¨Ò@ÉD"'Ô0?¢Žmìl¥E¿Ê¾Iý$-‡¿ã#³In¿ìXœ¿úÙ¿ï»x¡§Z"¿ïÔ+Á#÷+PSRPSR3FGL J0357.9+3206PSR J0357+3205?¦ôYOCãn?©Ð¦ã+?jþY?©Ð¦ã+?¥A›yTP?§¯pÍEä(?î«æH|y+?§¯pÍEä(?¼—éðbíÐ?¨xÞY¯LH?ìmÁó¢F?¨xÞY¯LH>7æ~âsI%>O_-Ú/¿?ïÿÿüÇ]Ä>O_-Ú/¿?}æsºc?€wX»?ïÄ3Ö=±3?€wX»?{ʒ)c?†|NR"
?ïÈjÛý'š?†|NR"
?¾t[©kk*?®/[;©¾?ì1tŠÒ'›?®/[;©¾=S¨ðºã?°='Î"àZù?ð='Î"àZùPSR4FGL J0359.4+5414¿êǍÄèì'?ìR«~H…UÀ8¢xíÀ;€k©œF@۔œê@öß$¾%j?¯!ÇÐ䉂?Ý»Ÿíp±@'"M‹¤
'?ø…ê ²?Ö×Yƒ)Ì?äêÞÐÛOG¿àá@!X?¿æx'vµi¿ïDJ¢Ž-¿ïÿü9¡â=PSRPSR3FGL J0359.5+5413PSR J0359+5414?Aδ,?>PžÄX¢?ïûŒRß ?>PžÄX¢?°{¦ÂáŒY?®(NõþÁ´?íð‹'ˆQ•?®(NõþÁ´?‹îp¡ØÌB?"µ6Tk`?ïF=jÞ_?"µ6Tk`??¥"´?2ë&$
Ä?ïü
î'Sá?2ë&$
Ä?@ö—͐%?G•z÷ŽÇ1?ïûÂZFâ+?G•z÷ŽÇ1?"èT(%ý?‰ÌÖ:'U¶?ï¬^¯Q«ˆ?‰ÌÖ:'U¶?ƒ_ÔÔ똭?dwSÞÚ¯?ﲀ¬sø?dwSÞÚ¯>Á \Žg>»9úð©?ïÿû·µ¨2>»9úð©PSR4FGL J0437.2-4715¿Þ¡CØ®´ÀDû† ˜'\À8Ǽ_—?LÀ<F…½CÃ@¿bå¨eå@lBHyì?¨žÕ˜£O{?à™ä½¯M‹@1ђً÷ð@Cå²÷º?ÂÉ·Ùö€û¿Ô$¼øÄL¿ãþ´;Œ¿í^•a¦Ž¿ïÿØ'sâP¿ïó?B5.¶PSRPSR3FGL J0437.2-4713PSR J0437-4715?Œ÷[…{™B?"Ôª1"l?ïŒ"'ê›?"Ôª1"l?ÇuÙQ{®Þ?Ã2ˆRõEg?ê"‰«¡H?Ã2ˆRõEg?Á¢Ã=EÊ~?­^Sç@"?ë—O0®`?­^Sç@"?=ЕPQz?>oŽÇ¬Ù¤?ïüEý Ð?>oŽÇ¬Ù¤?z‡š'Xëq?tŽRu+e?ïÊðËsu1?tŽRu+e?ª<ÃÍò'*?¨o¹'˜?î\3Ã.›ý?¨o¹'˜?ÈFÇÅQ|?µS 6ÌÞ?éîN«¿a?µS 6ÌÞ>¦ܛ·º>³'윾?ïÿþŸÐé>³'윾PSR4FGL J0506.1+5028?åj­Ì'¦q@îcŠ	À:ÚD«*»•À<ÝR‹¾@ œKZÇ?þá='AŽ@?ÏÍseÓC‰?ïmß«÷@H±il«@"0ðÇ(?â
—Íç¿à¥Ã=×Ñä¿ÔÄAéã?µ¤Va
±à¿ìmc`!¨Ç¿ïÿ°_ïÉPSRpsrPSR J0506+50?¸b7@~¸Q?Áì¨üZD?ìó¹¹/6?Áì¨üZD?ËV½âñt?Ä^Ð÷:è?é*X‡C£?Ä^Ð÷:è?×Z‡Îž'¯?²s
9,?äR¼°·)?²s
9,?ÌXœ†*sh?«Š6¡9½?èéØÞuc&?«Š6¡9½?Ã4¼{­Ã?Ê
Ïa
Ì?ë2Ðᾏ?Ê
Ïa
Ì?¿zØ"W?¡ƒç˜ò?ï)Zl]?¡ƒç˜ò?Ùˬ³Ÿ!?´_±ÁX¥?ãxš)¦0p?´_±ÁX¥?"m˵u˜3?‡Ùrû߯µ?ï\'¢™n?‡Ùrû߯µPSR4FGL J0514.6-4408¿Ð?ÔR
z"ÀA´^=¢ø¾À9ôËbi¤À<EÌòŒyö@Õ÷É$̓@X2%ìù"?¹R"¡?èԜ9‡
K@#W>«6z?ûÝr~øƒŠ?ïëý^åé~¿Ï͍çߢ½¿æhþ0Q׿ð?ð¿ïÿð ¼x—PSRPSR3FGL J0514.6-4406PSR J0514-4407?µ~¦	?¾8Ê õîÚ?í_+s?¾8Ê õîÚ?Ø
†¼êy?Ѥ{È«Þs?ãúö<¡ŠÄ?Ѥ{È«Þs?áUA,	2?´íÕAá-?ÝU}§íçœ?´íÕAá-?뉴_Àý?ÅóŠ%³?ÁÙ/¾€ü?ÅóŠ%³?Ú¦ð<ÇP?Ð|‡xboê?⬇áœxØ?Ð|‡xboê?´ÏZ5î?·Ÿ6'Á?í¦•ýò?·Ÿ6'Á?æDדi?·ï¯]¢³Ï?ÓwèPÙ-Ñ?·ï¯]¢³Ï?ÅÍ«øº?ÒÙ |Þ?ꌕ:AøÑ?ÒÙ |ÞMIXED4FGL J0533.8+6800?îû#	DwS@2/À~à°¯À9j1ZëÞáÀ<`qªm@YZô˜B×?ý¢"#æ?²q¬?¹~f?×áäù~@#ûb(E@ÒÿZh¬<?ï½(êÚÔÍ¿ÓßZÃðÛ¿Õ³Üȃ<¿àŸÔçM"¿ì4 ñ|¯¿ïþ SPSRPSR3FGL J0534.0+6759PSR J0533+6759?€o7a"]]?"ÖÇ¥ÛH?ï¾C"¥­Š?"ÖÇ¥ÛH?ÃgM?¤s?¿gøêÄÚ?ë&,°?Öã?¿gøêÄÚ?ºb¿Š;z?§;AB8?콨¸'?§;AB8?¯°ZÅ4¨?šÜ€tù_?îúV®ô†?šÜ€tù_?k~9‡d?nOwÉO"¶?ïäàÑw¾?nOwÉO"¶?¢î=RƒÌ?£çtïÿv?îÑLœs?£çtïÿv?—4Æ7?'ÿþ"S?ïF_O=L^?'ÿþ"S?`h"hõš?VËwéú~?ïï—lî•Ê?VËwéú~PSR4FGL J0534.5+2200¿æhfë5\rÀ ž³´ÎÀ4^ZXTÀ8u~¤˜Ñ@q?%3@¬À½ÊÑ?'
æÒ(ú?Êʖý'<@@ñ«!Z@GP÷iY¿É§•ßbÒ¿ÝÁíz—¿ãÑÖ!	e¿åÛ£>Þâú¿êô~ø-£§¿ïÿÛ¸"ÝPSRPSR3FGL J0534.5+2201PSR J0534+2200?ß]n¬AM?ÕJûY…µë?àÑH©ßY?ÕJûY…µë?§á×)Ò´?¤;Èð?îâuÁE?¤;Èð?Ü=
Jç?µ¾%!‡1?ááyZðøŒ?µ¾%!‡1>x¡é"Üe>†©`Dß?ïÿÿ˝Å>†©`Dß?ÈÎ" œuË?É\Èß=£á?éÌwWØâ?É\Èß=£á?wó9"ˆ?èps…à·?ïÑôuz‰?èps…à·?ÕÅכîïž?Àïç;…B?å2ˆ1?Àïç;…B=pëx[°ä2='•|f?ð='•|×KPSR4FGL J0540.3-6920¿ïÃëóa>½À?€¦—®ÞÀ8Pè¬&dÀ;1u§L	Ä@¸Ttvt@õV#"Cø?¥²žù)ø?ÔÆöôév@ ⟜èÙ@µ¬;ç%?îu×Ra̤¿änìF嗟¿ç	#•0~M¿çñbXdÆ¿ì6§â1¹¿î¤ZÝò%PSRPSRPSR J0540-6919?âæÿ V?Ñȴ܍?ÛÜ2¿SÏ?Ñȴ܍?Ö\«ø–Õ?ÉRì˜çdu?äÑó*´•?ÉRì˜çdu?äæý¸Rx?³æE³'=?Ö2[Ó?³æE³'=?Ðt(B¶«E?®!6'kÛ?çÅëÞ¤ª^?®!6'kÛ?ÄØb¬?Ãʅl2zž?êÉç|üTû?Ãʅl2zž?¹O8[íåÂ?¼µ­OÈ®õ?ìÖôKIˆ?¼µ­OÈ®õ?àv±G`;Õ?»&®%ÓàN?ߝq?ˆV?»&®%ÓàN?¼¸¯=ؙ?n•=Gé:?ïÀ†Ž¶!÷?n•=Gé:MIXED4FGL J0554.1+3107¿ïÿ¹ÛÐÃ@±@ìFÀ8²¥xÊìùÀ;êʉüm¤@Áj‹@êPÖ²(Ý?­áÀ,ˆþ?â+`kz¢^@+ýxÄ6ü?û£Z'"ÂÀ?ƒ¢=×üÖ«¿À.²šò_.¿ÝôÌÆÐ&¿éÞÿQš¿ïÿþBe«+?È^9Tš6PSRPSR3FGL J0554.1+3104PSR J0554+3107?R«'#êç?aÑ&¢Mì¡?ïöª7»G?aÑ&¢Mì¡?¬Œé…ZÁn?©u§ƒßj?î71g™?©u§ƒßj?§k£èØ.?šÝ#º¢ÜA?î‰EÁ€=}?šÝ#º¢ÜA?A.¯+Vcó?8™_ êÛø?ïû´T8š?8™_ êÛø?Iø<4E!?F_@›?ïùñ(Ä?F_@›?'yoìÏ5?ˆõ±³Æà\?ï¶@{?ˆõ±³Æà\?ÎJâbœi?¢Jý.0k?ï€ÆÔ»-¾?¢Jý.0k>¶¡G튰>·ÙÐE ÿ?ïÿý.rê>·ÙÐE ÿPSR4FGL J0605.1+3757¿Ä˜ÜÒ¡@ 
ˆ~¿#À9ÃÕ>ì¥À<'	µól@5&ƒwnL@ÖEüc"?»×²?>Ÿ?è¬kbNª@#ú<B¦m½@ý©¾Õ¾8¿ê§¼r¶?ï쎞"Ô^¿ÑU+@ªÀ¿æthAÝÅî¿ï{û#!m8?·!¶‰PSRPSR3FGL J0605.0+3756PSR J0605+3757?\ï"´¸?m~ú8@:?ïñõ]Ð?m~ú8@:?·\
͏?´k¥Q°7?í~FyX~?´k¥Q°7?º<Eá*?¥‰»nU"?ì¸w_cÛ?¥‰»nU"?'8³U™?}².´F	Ï?ïn?>'?}².´F	Ï?Q‹»|ƹ³?PkP%b?ï÷:"u›?PkP%b?Œµ‡M÷
·?'
û}Í"?ï)âã µ?'
û}Í"?•aH@÷Ç?'*˜*á?ïTõ½ÜÄç?'*˜*á?1#¶ËŸAš?"QüìÀàö?ïýۉ9`Z?"QüìÀàöPSR4FGL J0610.2-2100?š#Ƙ 
À2.8ÅCÀ9¶òÔô¹À<cÅü-ã@LÏõv9B?ÿÍø`ÏM±?¶žÕ)g­?àB««êÔö@"%p£×
=?æ'rhÓ(1?ïû®Þ¿×UÌeHÚ¿Ý+'€Íoà¿æš._8õ•¿ïÿèM[Óe?è:Î*šÞPSRPSR3FGL J0610.2-2059PSR J0610-2100?'ñ'ÊŠŒ½?¯ór´}~?ïpsií*?¯ór´}~?Æl$Ÿ?ÂÕal'¶?ê~ü$ܶØ?ÂÕal'¶?¼¢îu¾€?©Rq …"Ú?ìk¢1\ˆ0?©Rq …"Ú?‹8É3àä?|"'ëŸâ?¤6½?|"'ëŸâ?¡cᡧ!p?ÁKŠu—å?îéÁ懩?ÁKŠu—å?«f$ֆÜi?®mô"œÐ?îI²¥P©?®mô"œÐ? JÅ 0!0?"W`üÿvl?îûS­üýí?"W`üÿvl?'$Ž`°?%°Ð+[r?ïþ¶Ù½Ã?%°Ð+[rPSR4FGL J0613.7-0201¿ïïA¸X2À"œ-IfËÀ7ÿ6)‡¸ÇÀ;…ë¾íç@¢fè¾Æ@#¹…È+}? Ñê¡|šŽ?ҁÝ$Þ±§@/Qߗª¬?÷ÚöE¿Â1êžCøR¿Ôœ¼C'¦á¿áTaì""9¿å8@Ž:–¿ï
žT}‹¿ïþ{›Ñ&PSRPSR3FGL J0613.8-0201PSR J0613-0200?l‹õWŠŸd?m¬Çà)c?ïãt
¶3Ñ?m¬Çà)c?²ºECë
?±ˆ©‰á¸?í¨·W«É®?±ˆ©‰á¸?¢£Œ{gÄ#?œ©\|¥?îÕÇ8Iƒ¾?œ©\|¥?2ûs§{?1Äêb?ïý ŸrK¢?1Äêb?zñÕE›Xt?¡·ù#i|ö?ïÊU˜…??¡·ù#i|ö?ŽþZ¤Á^è?"nå^CK?ï"•£ôD?"nå^CK?‡Ø¼S´±C?z¨ôf"?̪?z¨ôf">¤›Ïh>°¤Ô}•
£?ïÿþ¶\{Š>°¤Ô}•
£PSR4FGL J0614.1-3329¿Ånû¢ð|ÍÀ5Óä öñÀ6åʅʯ¼À;7Äe>Š@æ]êÁÕM?ùkâqy¿ß?Ç+?ÉÅ?ÒÅq"tI@Db0<î?û‡"»c¿ø¸°W™¿§¶™bDÌ@¿ÕoiÚº M¿àz4CÔk'¿êD_½Õ¹¿î>¾L‰"PSRPSR3FGL J0614.1-3329PSR J0614-3329?"¶Êû?•PïžÃUÿ?ï_/"WmÐ?•PïžÃUÿ?¬6³Lµ"?­×¾0fu?î<"Îâ.f?­×¾0fu?ÇÛALÚð?°ì®Gœ8ë?ê	/¬ÉÄ?°ì®Gœ8ë>
NF¹#þo>*
ص7Ì?ïÿÿÿv¡>*
ص7Ì?wéÔ=±Ó?qÌ ú&o?ïÐ,W™;r?qÌ ú&o?…{®Æ(M9?Žðq,Šð?ïªEš?Žðq,Šð?·¬¶y…?±3Ò¢´&a?í
}[í³ï?±3Ò¢´&a=FT1ÆÉüy="RŒ¨?ð="RŒ¨PSR4FGL J0621.2+2512?̼÷dQí@L–F(~À:õ۹ϚÀ<'¡Îò@û@ˆuZ 	 @mYO&®À?ÇéKó?ïÿÂWþė@ öHÇ@±B%¿â1؊p0ë?ìœÏCŸ'?¸¸Û¾­$f¿ÝèŠBŽšã¿ïìü‡7¿éL"b¥¼"PSRPSR3FGL J0621.0+2514PSR J0621+2514?ˆÊnÛÛ?ªý Ë©A?ïœÖGþO?ªý Ë©A?¹wl32q?·)!=e²?ìѲ¢Õ?·)!=e²?Ç-²~ž4?«Ú1˜ÝÃ?ê4"`xs?«Ú1˜ÝÃ?ÝbŠþe?r-h«T?uÔl?r-h«T?¡÷ò1¹ ?Ƈ¤	ñ,?îà€Ý_¾?Ƈ¤	ñ,?/°§>…?"–D(´O?ï~'zÕD|?"–D(´O?ª·¤\T¦?œ‡:ß^{µ?îT…¹ùò†?œ‡:ß^{µ?CæãÐ
»?4ÅH¢Ü?ïû³¥?4ÅH¢ÜPSR4FGL J0622.2+3749?ïôS'ç@%òµÖ\À8ÍIï7ZàÀ:¯ç¯§"@ìáÖõÈ@E!Whœ¢?±qta{Æ?êQ\1Y@1p æ)•%@þ¢vb?ÛÛPޔËT¿Ð*~CQäN¿ã¤©,´"ñ¿î€úfc¿ïÿîÝÃÀ	?ïrbS—WPSRPSR3FGL J0622.2+3747PSR J0622+3749?p"Ó'ç°?ƒÑûùÈ{?ïÞÖXÖt°?ƒÑûùÈ{?ª´ó0F–S?¦ðYg?îT°ÌĜÛ?¦ðYg?·©S_ž?¤‰ˆV§Æ?흪þÏ\?¤‰ˆV§Æ?%³›œÝ?)È3ï?ïþ®u0?)È3ï?u'†4?vï&ê&±?ïÔúóü'Œ?vï&ê&±?'Œ"Š­‹É?ˆ_Æ<v?ïµÍ±›a?ˆ_Æ<v?¢N®Äç	Á?—Ïäá÷F?îÛÚÊ´?—Ïäá÷F>xæá0">ªO- Ë‹?ïÿÿÏ®~ƒ>ªO- Ë‹PSR4FGL J0631.5+1036?´nËÔ?Ý`IôÀ83¦AGÈìÀ;qc´~ë@[áþ@и,+Ø?©%œq».?Ø 1ί%@+"ê»Ë?üg¿	ў?³½ŸˆF
%¿Çdëýi¢±¿ÙdÛ·K[H¿á~®üØ-S¿î œ˜Q›¿ïû¨¸Ž!PSRPSR3FGL J0631.5+1036PSR J0631+1036?9É0—²0$?<ûÃæFô?ïüÆÙ²}/?<ûÃæFô?®^uír'È?¬bžKS<G?î ñãÄ?¬bžKS<G?‹e!ö?‰Ü'@oXi?k¢÷x?‰Ü'@oXi?BTfD(!˜?8Ç|–ׄû?ïûjæ9±?8Ç|–ׄû?Mˆ"–]p
?<Ÿ4-'à?ïø÷ˆsh?<Ÿ4-'à?'®¯>À.Ø?‡"	x.â?ïµEBïÅ?‡"	x.â?"®¢'8?qÏʊR«Ö?ï­Ewоk?qÏʊR«Ö>¿Nè\šl>Á(T+g4?ïÿü2é¯>Á(T+g4PSR4FGL J0631.8+0645¿ìcù-ö)à¿óêwTË3À8æpÆ;¹À;©´oÞµ-@Ây5v'@XºÍÆÈ?µúaŸF°?â.,Þ°O@"±P¹U÷ƒ?öT÷™Õ¿éâ—½#â?x6ŒGæ7¿ÎÁ ܙs"¿Þœ\W뉿í´bþQÿý¿å֔APSRPSRPSR J0631+0646?b\±'@?gàyJ[b?ïí£O-˜G?gàyJ[b?²êØ5­ó?±pÓ8u+?í¢¤ù&Ђ?±pÓ8u+?©Xµj-æÛ?›;†í.<
?îjt©†\â?›;†í.<
?tޘxȘÕ?^µë–ßӁ?ïÖBÏ)ë®?^µë–ßӁ?‹Â¶À¾C?ºëê|é"?ïõ$ýô?ºëê|é"?…iI$2ê?ˆþ	{kë'?ïªZÛT
T?ˆþ	{kë'?"»Fd(Ο?‰²Fü£0?ïb%ÌÃ<«?‰²Fü£0?ô9h÷?ڍ'–µ?ïÿ/àø?ڍ'–µPSR4FGL J0633.7+0632¿ä)sÁI¿íµÕڒˆ-À7\Wï«À:¾çW'Ž
@W7•BœÞ@Oú Âî'?–{Ûî}̊?Øp;7äs@:@¿ã°>?þ;Ÿ]¨Ò?侏½wÅ3¿ÀfÌ}F§¯¿Üv" ‹Â¿å½ýûC¿íï@?5J¿ïÿäA2¥DPSRPSR3FGL J0633.7+0632PSR J0633+0632?:Ÿªã5™?6
੅u)?ïü¬
àXÆ?6
੅u)?§U£[Ëi?¥î/¹W?ÊCIp?¥î/¹W?z,u/~1,?yáû3ò³­?ï˧áœE?yáû3ò³­>'w[!Õ»Ž>š'=…œý?ïÿÿtißB>š'=…œý?KnˆÃâÞ?<M^ƒjdº?ïù$ÍPç?<M^ƒjdº?yÁ&¦?|¸ÿ:0F%?ïÌÞ}×Ͼ?|¸ÿ:0F%?'Dg
*_û?_­l§v¦?ï¶îcËV€?_­l§v¦=¼g¡,£ž=æˆÝMÆ?ð=æˆÝMÆPSR4FGL J0633.9+1746?íüý…b'+@‰I`œÀ3G9"†À9)`ì©áæ@ÄTÉ@gëC°Xù?hC˜ÚLª7?×&v î@l8²êò@µMÏÁžÆ?Àaäáìn©¿Ã2äá¿ÚD+]ÑÂU¿äØÍ÷o7Æ¿î>FVüf¿ïe<ã.PSRPSR3FGL J0633.9+1746PSR J0633+1746?ïž±äó?¤ëK;]f?ïˆCÅ@€=?¤ëK;]f?Žù¼øø}?ª"H¿*…Œ?ï"y"^?ª"H¿*…Œ?œÝ¡e¨ÁÏ?•9ZEšÂ?ïôàxa?•9ZEšÂ?ð?y¿ºªà7¿?®±ž'…Æw?ï̀Š"‰?®±ž'…Æw?`d·%é?yÀ6ÉȆ?ïï›HÆBo?yÀ6ÉȆ?'<ݦÅÄH?_éÑIÇ?ïn –Ž?_éÑIÇ?ðPSR4FGL J0646.4-5455?ë3Nô¸À6˜>·Ë³ÈÀ:º™I—#À<å³Ët9@áÞ¸1µ/?ý¤Uêî ?ÇïÂǺê?íuÉ næ@›ò9?ýJk±ò?ïøö‹â÷±?É|)WIh¿€|Àò+µ¿å…ؼÅÍ¿ïü¶ŸcÝö¿ïÞ?állPSRpsr3FGL J0646.4-5452PSR J0646-54?¹´$AJD"?ÃRg[?ìÉ{wÖ·m?ÃRg[?ÓUC¥'ã?Æ#Tgz&|?æU^-6Ž?Æ#Tgz&|?Ñ]"9êB»?±¬ßp¹1­?çQ6c
Þ£?±¬ßp¹1­?º·"¬Iõ?Ÿg¥AÉÈ?ì¿)
jvÁ?Ÿg¥AÉÈ?µç¶x?Êå‹óÇ@$?íCý`a?Êå‹óÇ@$?´lä&R?µIã~?í|ÿ²¨3e?µIã~?¼y
˜_\Ý?«ªcÂ!l?ìpÞ¬ôd?«ªcÂ!l?"@(›Úä?uLJc3þ?ï®ÿ_¤³Ý?uLJc3þPSR4FGL J0652.9+4707?íIñNº@3¡/À:íu¶e';À=ÊC…Î@¾~ÜÿÊÑ@¥ð¿ñ7?ÒI·¤F›Æ?ïÿ³ß•ý-@[Ha˜¡L@,a$Wοã?ǖ,'?·†M¡sÙ¿ÑÄÌběP¿íðqJ¿æ´|¿Y=?–·Íûå­ÞPSRPSRPSR J0653+4706?ê6Óóÿä?É4Ë÷îAD?Ç¿$°0p?É4Ë÷îAD?áÄNÿË~?ÊK5Ý\'?Üwbi÷?ÊK5Ý\'?å  {'é?²³FPØ«?Ô¿¿	âú-?²³FPØ«?áÛ9››ì?³U¹>"T$?ÜxɌÈÈ(?³U¹>"T$?ـÔ+:ì:?фËн6?ã?•êb‰ã?фËн6?µ_"â–%?»pW/UœÙ?í\Ô
L³|?»pW/UœÙ?ÜP<…ŽÂ?¼&¨ÿEÎt?á×á½8žò?¼&¨ÿEÎt?­<Â
ùnœ?–ñL­Ž?î,3ßoW?–ñL­ŽMIXED4FGL J0659.7+1416?ïÿކwl¸@ ‰3ÁÎl	À8U×øyùÁÀ;¹SšÍv@ÝœRÜq@§-ä>ÙZ?§¾Ûrýœ?ߏã=Qš@)vB||R@}¿|ØÚ¿±A)¶2¿ä°Iÿ}y(¿ì~ð€±a¿ï4mÙw¿îøÛH'¿ï§­Ãó	wPSRPSR3FGL J0659.5+1414PSR J0659+1414?–a"oŽ-U?°ìézg>?ïLó\ÈFÅ?°ìézg>?±Ea£9ÿ¡?¯5¸Ø$ùò?í×S˦~|?¯5¸Ø$ùò?Ù<}œz[?³*\m¨ÊÆ?ãaÁ1ýÂÓ?³*\m¨ÊÆ?n>.í³â?ch¥½â¢?ïáÁÐç°ö?ch¥½â¢?¿Èbk]ñ?ÄÑP†‹û?ìó²TB?ÄÑP†‹û?"$`–~?ˆê)øù…Ð?ï¯nåhz?ˆê)øù…Ð?ず´Ì¥à?³¥zÌpf?Øüʖf´??³¥zÌpf>æV'®——">ãÕîî‡Éˆ?ïÿé©@D'>ãÕîî‡ÉˆMIXED4FGL J0729.3-1445¿à«ò™‡rr?÷x¡Åg~À9Ä÷øËÀ;|rïá¤Ë@§>9Ìu@÷µ¼g?Ä1§—ß]?Á°å^"
?ùÖ‡å</@c‡8îß¿ï,ýäò³?ì-Óbh*¿ê°ü¢'‡®¿ã\áb0!¿è´y"P\9¿Ü~ÒÃܹ)PSRPSR3FGL J0729.7-1448PSR J0729-1448?ïôyaôDi?…Ñ	ë¦?W
;ºÏQ?…Ñ	ë¦?ïÞÔ7¹ç?wcÅ-»^ï?p•ð`³pœ?wcÅ-»^ï?ïÈ[¯ï?|-¦·Pm
?{Ò|/—š€?|-¦·Pm
?ïÑC÷Hé?[ßÝ5Ó´?w^:÷˝?[ßÝ5Ó´?￈˜·¾À?"*¥Z?€Ùƹš?"*¥Z?ïåfC‹?ªa˕øÌÆ?œ#S)8Vµ?ªa˕øÌÆ?îxQ¦Ìï? @Û´¾…"?¨z吝Yˆ? @Û´¾…"?î¼Ûù™<?'FøëlRÂ?¤2@d·A?'FøëlRÂAGN4FGL J0734.7-1559?íM:‹Ê¬•@')óÀ7Ít9ÀÀ;:¯ åS@³ËÉít@pM•ö?¢ž©_¨ß?ÑÒD2^ø@,ëXK±?ø¨©—h'忳ú§ü^¿Ú+ÎÛ쐿ã·'hÐy¿çpGüó¿í+/#:G¿ïÿå"m/®PSRPSR3FGL J0734.7-1558PSR J0734-1559?uÀÍ#چ¼?sk†EÛS?ïÔ~eœÎ?sk†EÛS?ªÐýMʨ?¥d"ÁÛ^?îRð'oۅ?¥d"ÁÛ^?¼n	%¡,é?©—‹—5VÈ?ìr>ÛKÚc?©—‹—5VÈ?C'6iåG%?<s;2\h?ïû62¨/?<s;2\h?hYJüü:?_›µnW?ï禴ׅ?_›µnW?~à0·læ ?'RY ¨ +?ïÂ?ž·¡Ô?'RY ¨ +?›‰!™†8?–×E%'?ï#¶ó
'ð?–×E%'>·û%YP:Ð>€çP9#?ïÿýϼI>€çP9#PSR4FGL J0741.0+6618?ànªáÔÇ@=ŸØ{V¸sÀ:{ÑEØÀ<›'BCJ@͜ùöPª@
U£ ƒ™?½Q°vÕÊ?ÕR%'@Ôà—"ì@3bt>kK¿çT¶:º¿Þ*ƒaHð4¿Û‹ç)oe¿ä'£+Ó¿ì–ÿ'èÒ¿ðPSRPSR3FGL J0740.8+6621PSR J0740+6620?ær8^7»%?Å>ìJ§ª:?ӏC‰·?Å>ìJ§ª:?î
!ÿ»"?³æïÿ"?¯-ﲗü½?³æïÿ"?ãV©‰Ét?´ã0éZ?ÙR¬ìmã?´ã0éZ?ííénO5?‰ÜÆZñà?°·ŠÕ¸W?‰ÜÆZñà?Α©*†;n?é+p,t?è[•µ^q%?é+p,t?äB.£¬m?΋n.m?×Ó{¢¸§&?΋n.m?Äќӓn?±¬ß'µ?ê˘Ë$|?±¬ß'µ?ãl\ýå|?´u¹¿¤§1?Ù&åF5?´u¹¿¤§1MIXED4FGL J0742.8-2822?Ó-­€^è¡À‰p"XðÀ8êÃ×ZÅHÀ;¶–F(~@&(Ûì@è&ªŽ´c?±vÊâ'Û	?Ôýåÿ"àU@Ôñ€
|[?ýd"äÖ¯?êV?rÖÚ¿²khó¥T¿âTB)Æ"¿ç¡Y{•£¿íOx¾'²!¿ã#͚R&>PSRPSR3FGL J0742.7-2824PSR J0742-2822?¦%7´§æ?±ýoÙ¹ß?Ž=ðÑ?±ýoÙ¹ß?»£×—ùRß?·€¤'MD#?싅
Õ¤?·€¤'MD#?ÃPA¥«?«ÍS2ìŒ<?ë+ ?«ÍS2ìŒ<?±Ü(¥ß¤Ë?'ññ…¥?íÄzë{&?'ññ…¥?Ÿ r'Ö?· H¶,kQ?ïüo8a?· H¶,kQ?}àœ±O?—ÃMR>?ï'}tl[?—ÃMR>?¥} ¾Æ¸?''Ô[³æ?ïzÔÃ?''Ô[³æ?[^;¨Ü?H×ÇN‹?ïòPõæB?H×ÇN‹PSR4FGL J0751.2+1808¿¶ÁAþº÷@5‰Å!ÞÀ9]oˆN»À<mByø¢@éR&ht‰@;ÔÂe?³²- ]iN?ç@Íàžö@+€Ïž8e@‡ùw¥¨ñ?ïÿ½OG"?驜œ€¿Äüì$Uõ«¿áà«aG¿îÉ=+¹É¿ïÿÈ¢› ÛPSRPSR3FGL J0751.2+1806PSR J0751+1807?@+ý£ö?IÂ|Ô
Íã?ïûõÈ|Ü?IÂ|Ô
Íã?¾m…Р'9?»ùñªýš?ì2OEëû?»ùñªýš?¥"©2hí?™†Y/xþ?na\'?™†Y/xþ??üÁ§jÀ¦?4võc!rÖ?ïügÀè?4võc!rÖ?Z<ŠŸ~©Š?aMS_ÚÒ?ïòáºÖ¼K?aMS_ÚÒ?™ÊöTýÖ?ž€{%ë@
?ï1¯˜Ÿâ?ž€{%ë@
?"®yº&
"?fâdjú?ïbŒ2"G?fâdjú>Ç]qD;A>Äّ£µ?ïÿú(Ѓ¼>Äّ£µPSR4FGL J0835.3-4510?î*ÑØØÒGÀMCš‰ƒ¢À2{Èxª5ÉÀ8AA [À@ä¥}'ÿ@_ø"»ì«?gÖƒX/Y?Ô@Àæ"t@j¦[[Õ?øG>¾×?Ÿ
fÞõ¿Ñ``'çα¿àQúž—/\¿å£~IÜî¿ìö
Ù–ó¿îϼ5¥Ô:PSRPSR3FGL J0835.3-4510PSR J0835-4510?Huu9ËM?UšFö1?ïùø¢q7-?UšFö1?'{ÉAUt?š2•³Ã×Õ?ïwT!Œº?š2•³Ã×Õ?‰ôë¯#	>?/PËàÄ?ï˜,Ql¯+?/PËàÄ?ð?EsE‹Uœ£?LY`o¼c@?ïú£.e:?LY`o¼c@?dxkR/¶ö?sš¨?ï뇔x6a?sš¨?'¤÷,²ª?Xª"5gÂ?ïµl#rS?Xª"5gÂ?ðPSR4FGL J0843.3+6712¿ï¦'ÍǕù@AÍÀÀ:hf9ñÀ<žSËY/F@Q¨¿&?û{Ɋ"-Q?¿-ý¿3?Þë¢ÐÏç@ªÉlÅü@Æfªƒø¿ç~è¾Dô§¿ÀB)Æ"¿ÆšXz"D¿×B¹ãæﹿé*æ}Íá¿ïðJ¶·ªPSRpsr3FGL J0843.4+6713PSR J0843+67?ÉJŸ>&à?È~"p''?é½-X0vH?È~"p''?ÜCK£[S'?È"FbSÌ?áÞZ.RVm?È"FbSÌ?Þ¸³¡h×?²Di÷À?ࣦ/K"u?²Di÷À?âÓ»fÑxâ?´1c‹
çT?ÚX‰2]=?´1c‹
çT?µÌ_-{Ó?ÇÕ]»	è?í]†t_µ?ÇÕ]»	è?·8e›<d?´TG
B³‹?íóLÏw³?´TG
B³‹?َ¢Ï<,›?¹Á=ü©£?ã8®˜aé³?¹Á=ü©£?¸ŸŠªît ?¢«I»ÓÛ?ììªxö?¢«I»ÓÛMIXED4FGL J0908.7-4911?ïâãóϤ¿ï™–òö,À8‡oó­â&À:{ýÍpa@XŒ­@C\ƪsÜ?»Ì뀗.?à—-¾ªN@!iÓpô@ ôÆ/$?ïo5ýè΋¿ã6oÞ_Fb¿å–Ÿþ7©¿ìtáMK¿ëî‰J–ý¿ïþ}ÿŠ9TPSRPSR3FGL J0908.4-4916PSR J0908-4913?QÄ.k?©WUF?ô¸N;?©WUF?²ºÎ©#?ªè¬Ö|ã?í¨¦=}L?ªè¬Ö|ã?Ä®>õ¼¸¶?¬Ìvô®1?êÔpBÑÒ?¬Ìvô®1?¡­n]ŒÀF?¸[3~óÖ?îå)^-»?¸[3~óÖ?ŒææÊ-?µgýJ†"?ïŒdd®€\?µgýJ†"?¿ìÈud-?'®o	
Gú?ï¹LߊG?'®o	
Gú?±pś…K?£ì@f"·ò?íÑçLfN?£ì@f"·ò?/ԂHþM?-üã©|Íp?ïþ¸Èv?-üã©|ÍpPSR4FGL J0931.2-1906?îŐ &Ę@78ÿûÎBÀ;Ñ‹èÀ=nda©h@@¸MŽÔ@ºÃ.¾Y?ΦKÄ#°ß?ïûK€1È@æ…ý¢ý?ø^ Ò]…l¿ì"Ì3?ïïWq\?¶Q'ľ5…¿çVü\'¿íü'Ÿ½J¿ïæ#뗓/PSRPSR3FGL J0930.9-1904PSR J0931-1902?­BãOQ>:?¿'	¯+Q=?î+ÑËAåÜ?¿'	¯+Q=?Éï€ã·—S?Ä-ãTÅ÷h?é"Ç+?Ä-ãTÅ÷h?ÑÒt°ÅÉè?¯çð®m*?çŧ?¯çð®m*?¥	ҊӍn?‡Z("Gf¶?î¯b×nD	?‡Z("Gf¶?Šu
ÃþG?šá¡±pCî?ï–+Ô«N´?šá¡±pCî?§6"o@Þ?©®\°kS?¹ò?©®\°kS?³XuÇÌ?±?£'·ŒÆ8?í"ñFÝ<º?£'·ŒÆ8?`zeÎWâ?P+Â½7?ïëh?P+Â½7PSR4FGL J0941.1-5429?ރr®M¿ô‹'!¬ùÀ8úH…ªÏLÀ;µÛSñ@Þ)–|Y@Kh¢×0?»–ûÁÖz?âüÖö@"§â?$Øý@«<UEצ¿ïí×Äw"?ïÝ̙¡&V¿×?›ÜÀ¿æ{:ˆ&*¿îgý?[_¢¿ïÿýFKêPSRPSRPSR J0940-5428?'–¥—€o?—dAsðm?ïkJÓQº÷?—dAsðm?³Ë,픅˜?¬'Rӂ6?톚b[-½?¬'Rӂ6?¼ûA>ä—D?§ãÜӓ?ì`—Ø#m?§ãÜӓ?±4zDº{.?–ٍ×Çx?íÙp·M3º?–ٍ×Çx?ƒI¹'˜',?®@f&§?ï²Ù9ÂD?®@f&§?'&Šd¼§ï?ƒ™ØŸç?ï·eÖYϐ?ƒ™ØŸç?²piÓæîø?¨êÁY›	®?í±òŞŸ?¨êÁY›	®?Vn'å·]²?GõM#Év?ïôȶ´ÿÉ?GõM#ÉvPSR4FGL J0952.1-0607?È¥!Óörõ@A±tÿ†]}À:È5šì€À<ÇÃqÚ7ï@xJ7[·@#3vO¶?ÇqØõÏûU?åÑneZÎ@›"ªNô@¼½{¿í½FG.?ï«᛿Î">ï)¿åû«©g¿ïÿþÐñ?ïÚ?›Ü?PSRPSRPSR J0952-0607?Ü0ζÔ4m?Í4a¤"P]?á瘤•åÊ?Í4a¤"P]?æÓUꏢÂ?È°­Î@%›?ÒYT*àº|?È°­Î@%›?ß<pPAƒO?¶¬ð‡*ñ?àaÇ×ß>X?¶¬ð‡*ñ?èî(ðLÚ?­5½
¾É?ÌG_°>̙?­5½
¾É?Á'½I¢
?À²tLê$³?ëŸP­—}`?À²tLê$³?ÃVuWšñˆ?ÁÁµJ,Ò?ë*bªCž?ÁÁµJ,Ò?´ÑÃèEÐÏ?¢×hYŠÕ?íeǂé‡v?¢×hYŠÕ?Ê¡úwž??µ˜aW?éW{bp?µ˜aWMIXED4FGL J0955.4-6151?â@Y[³QÀø*ùÀ9ª¨ââ¸ÇÀ;ñ롤*@ŠÍ²¥Ú@ ` SÇþ?ºCSyO?ÔÐ=ºË˜o@»­ˆ["@ۄl5Þ3?ïZ° F\¿Ñ,b´€%¿á/âjmÝ¿æ:"ÀÅ¿íÎôÅ9Z•¿Û‹<¿N	"PSRPSR3FGL J0955.6-6148PSR J0955-6150?ࡊ›=ÍZ?̈³d¾=?Þ¼êɄeL?̈³d¾=?ä&®Ê"t?ǬŠ¯hZT?ײޢj×?ǬŠ¯hZT?ÛÈX=¯Ó?µ­·É/‰[?âÓáq¨?µ­·É/‰[?è|üŒFä…?£âÓ
³Ë?Î
Îämí?£âÓ
³Ë?Ÿ\(\Ûò0?žø'ѽó!?ï½&ÞÞ?žø'ѽó!?ºô
ꊉ?͉ÎÒa?ì¡~B®®Ý?͉ÎÒa?£H Mf?˜Øjéª?îÎûvê~J?˜Øjéª?Äæøì3?£â
B1œ?êÆAÄà3 ?£â
B1œMIXED4FGL J1012.1-4235¿ä;OŒZA@&u֝0'À:ˆ­¹OÀ<u¦N³Â:@,mÇ-Ñ@PwFˆz?¸c±€@,@?Ói^¾Q^í@»hH¾µ³@¬OТÅ<¿Öc[ïêß¿áöуòÖ¿ák#>ô\‰¿áSµõòð¿î¹ý‡»¢¿ïþ÷÷óÂPSRPSR3FGL J1012.0-4235PSR J1012-4235?ã™ï¦|½&?ÊN>º®oÈ?ØÌ ³…´?ÊN>º®oÈ?西R÷Û?Äí¯®·kš?ÏÝi´ •?Äí¯®·kš?âËuØ«A?µm–(Zn	?ÚiðN©~?µm–(Zn	?ìââ&¿÷?—úÂDâˆ?¿ÐèîÊG?—úÂDâˆ?³çÌmÒ"?±
Í<òS?íƒFVÈÜ?±
Í<òS?Æ;3tvŸ?Æ9²Q)
?êq<s"âX?Æ9²Q)
?É	¾žûr?±n_—àÉé?齐XA#{?±n_—àÉé?ÕioŽÙ!?³0 ÷Iâ?åKwÈ8"o?³0 ÷IâMIXED4FGL J1016.3-5857?Í
'ºóË-¿þõ™t°¬À7dÿŽÀøƒÀ:;ƒo‹©@>ôŒÚ@cäõ8?©)·ßTä´?Ô°ß¼ÀL@$ŸÖ¶Zš€@'ð,¯?âã-ÌÁå?ç.ãBZ¤¿á×ûnÕ÷¿ålÚß4-"¿ì3Ô
2îj¿ïÿÞÝpˆÿPSRPSR3FGL J1016.3-5858PSR J1016-5857?gewö«c?"ÐúÙx?ï蚈#qì?"ÐúÙx?¯Ó¶Zvld?§›ñŒ?îĚ=Z?§›ñŒ?Ÿî–~òI?—ÏßéĆ?ï‹OBÍ?—ÏßéĆ?z¬¹š×ù?lo'†Õ?ïʦ¯à?lo'†Õ?j5b¶L8ƒ?¤î² ŠJW?ïåʝ{.'?¤î² ŠJW?æøKCˆà?'Z9]°ú?ï¸dÌ?'Z9]°ú?‡nkÉ«?{ÀI[¬?ï¢G¢ߔ?{ÀI[¬?

Î:‹ÿ?áXwb=ú?ïÿ—ËõG¦?áXwb=úPSR4FGL J1019.8-5749?ݽÔü
¿åþ-BƒéÀ8u2_Μ±À:'
´©@ÿ¦|V@¬øCsW?¹Ü<ŒAí?Òhm
&Ú@Ýø?A^o?ú[çW´³?ï…/‡­¿è³ÿ ‡	¿ãíê‰v5ç¿ãØÇ«â¿ì:"å$²g¿ëDõÓVTPSRPSR3FGL J1020.0-5749PSR J1019-5749?ÕäÈROê4?Î~îh0Ÿ?å
›ÖØ
æ?Î~îh0Ÿ?Æ¬´‡Z?½ÛŽØ0¿L?ê|ÔÒÞ<i?½ÛŽØ0¿L?Öà'ÿ'?´d'¡?䏾ýq??´d'¡?Áv;s#?£ºfrï™}?ë¢q9Ü£7?£ºfrï™}?³a2Iÿ'"?ÇVY9=t'?í"Ù¶À?ÇVY9=t'?Ž|Žµ©´^?u2	§"?ï†
Å)Y/?u2	§"?º³"ù÷u?®'m3ØÎ?ì½é› Á?®'m3ØÎ?j§s½)?XËìèJ&?ïåX‹ÿŸ?XËìèJ&PSR4FGL J1023.0-5745?®ž°ý¿Ùv0¾ŽÆ'À6¦|µ]DÀ97Ó«ä@•#/Úä@W†Üþs8?¢äý› Ø=?ÖÐ6
Ù—@3hî9.÷?ön¼ÆÅKÏ¿Ì,û¡ ¡‹¿Ø …Üxfn¿ÕMý¹Ô¢"¿èq_=Ó¿íÇHɝmd¿æýsþÕ]•PSRPSR3FGL J1023.1-5745PSR J1023-5746?N5¿¢µì?a•.C=ü?ïørênH?a•.C=ü?¨´2ïbñ3?¥&±5:Ì?ît¼Ñ	Ðí?¥&±5:Ì?¦®!"ˆ€?œü-|SÒT?î•æðºh?œü-|SÒT>̗<PFÏ>ϏwæÒä¤?ïÿøÚXì>ϏwæÒä¤?cˆňzU?œVòkÓõ?ïìwó¾?œVòkÓõ?|F·¶}?~W¼+IAÙ?ïÇ×rË­?~W¼+IAÙ?‰tEßùži?z¦ŽÃ™?ïš.è©TÖ?z¦ŽÃ™>'lJ¢×#>s£Ý´?ïÿÿÿv¡>s£Ý´PSR4FGL J1024.5-0719?î.슊æ@D?_JsÀ:&­czù›À<nÌ¢Ûa»@²r'å¢?þ6"çƒ1x?Á …¸Ò?ÛÛO\¿l@Ô»ó¡M@'´ªA2?ì<+)yv¿àš®×ï?¾¿ÖrÆ{ÏÚ¿ãfŽàV¿ð¿ÕÉg}ΊPSRPSR3FGL J1024.6-0718PSR J1024-0719?Ûf
	A¶ó?ÔOš˜®Hd?âLù{_$†?ÔOš˜®Hd?á8¬à¯hõ?ÉdÕ(CŸ?ݎ¦>¡.?ÉdÕ(CŸ?ÖX3ÚðHt?³[xYkf?äÓæ‡ÛÆ?³[xYkf?åM6éd÷À?­µ‹´öä›?Õe'-6€?­µ‹´öä›?¶¦
|Ùåý?¾-ƒ±ƒ?í+>°r°?¾-ƒ±ƒ?¹ò²‰ËE?µ'å¦w?ìÁ©®Ɨ?µ'å¦w?²éI5
?¢Ø¯I¨A\?í¢ÖÞbe??¢Ø¯I¨A\?¿ږ9ï?§kí‹t—ö?ëP	Zq»"?§kí‹t—öMIXED4FGL J1028.5-5819¿åö¼¹šR¿ßz0ÓJjÀ6
\ËOÀ9ëQ=à5_@J.%'E•@%Uœê†ò?'Z,œ@=?ÑO>šõ@<g†ø­?ûð¢l¦òH?ë\âŽÕñ9¿×•Ù[%•'¿áåNšDº¿åu'¾´V¿ë«ä<U¿ï$à>ï~þPSRPSR3FGL J1028.4-5819PSR J1028-5819?r`¦¦ù?¡Éü+Ú&?ï'6}.mÀ?¡Éü+Ú&?¨B8i?¥•

œ°?îN›³>?¥•

œ°?©Ð>J­<(?Ÿó€2éÑ?îbüt?Ÿó€2éÑ>rL…uù~·>/c˪ ?ïÿÿÛ~&³>/c˪ ?xìdM®?®²Z
Ü~¦?ïÎ'7Hãì?®²Z
Ü~¦?yd! ê?}4‰¸k8?ïÍ7ÁÀÝ´?}4‰¸k8?"»<™Ò7?pÎÛ×í=?ï­
pMg?pÎÛ×í==€z¹ðf<=ž6s¬,€?ð=ž6s¬,€PSR4FGL J1035.4-6720?̘ü%Tù,À`n¹ªÀ8µØGTRhÀ<µ™ª`'@Œ<‹v–4@ÿ‹eú/Ü?©Àc‡ä»?ázM£÷Á@0o¸dàT?ùL•Xí,?ïöÎ}üÛ?͔àwN–¿ÖZÆ?iøA¿æžvx,¿îjÃê¥ü¿ïÿüoQÇsPSRPSR3FGL J1035.7-6720PSR J1035-6720?PìĤ‹?Y=ZÑJFˆ?ï÷ÀtŠý†?Y=ZÑJFˆ?²8x²zXd?²bùÔ<¹·?í¸ðéÙðC?²bùÔ<¹·?ŠRÏ禛I?'gѕn??Ào$?'gѕn??Ä«äïý?úY³ìó4?ïÿŒð
`ù?úY³ìó4?Jë/ߋcÛ?>È%Ç}¹R?ïùE3Ä[B?>È%Ç}¹R?‡Ý‹×|7»?M#æ[Œ?ÐxÓÑ?M#æ[Œ?…œÚawù"?p5¶t¶€?社–PäÊ?p5¶t¶€>uC¨	‰v=>|ÝJe1±?ïÿÿՖR›>|ÝJe1±PSR4FGL J1036.5-8318¿ì JhLÀ5'"»äG=À:Dã)/¤2À<‰æ¤å'7@óú0ÞP?þÿ ÜïYÀ?½ršÀúËR?àЍK­}|@Ž½'¬î
?ãq÷ÝØÊ¿î7ûþé?ïýÖZHŒ¿Àí ÂWÓÑ¿æ6™ºPÉF¿ìDŽ#ρ¿ïÿ®¡hšôPSRPSR3FGL J1036.0-8317PSR J1036-8317?¿VEÇ_z?Æ°ùG)4W?ì7G®?Æ°ùG)4W?Ƀi\÷
#?ó<¼ô¾?éŸ%¨Â<·?ó<¼ô¾?ÈwUµFÑÔ?¬RCm¼?éâ*'®K‹?¬RCm¼?¢¨>ip|­?Š­S@áõè?îÕ|'3…?Š­S@áõè?­Žßɂ)5?ÆZÞ./Nˆ?î'ž×,?ÆZÞ./Nˆ?±TÔ;]?´Ôc&¡ ?íÕ|%aÛµ?´Ôc&¡ ?¢ö¸"æÄs?"Y˜¬ò'b?îДv³ÕI?"Y˜¬ò'b?QãCƒ?DddLXÚ?ï÷^‰ð|?DddLXÚPSR4FGL J1044.4-5737¿èÇztT)'?ò€]£IEÄÀ6õ€ø¸ãâÀ:jýKð™[@Ôä'±@ΕY˜øŠ?œËux–Ùe?Ôb«Ü<Vr@4B†ƒ<`@J€y·üÜ¿¼3@®ñÅ¿Ûv·¢CC¿ã9Â~•1U¿ç
ŸÎ¿îYD_*‡é¿ïû•"d~PSRPSR3FGL J1044.5-5737PSR J1044-5737?cr—†HËÍ?fCaN-›S?ïìhDL?fCaN-›S?§ÃÏr½Ž?¤J.Ìl
Ý?îƒÏ'ߘ×?¤J.Ìl
Ý?£ÃkUnÆ?›6éU'E?îÃÉNÏ,4?›6éU'E?ñ2.˜í?	`ï5ä}?ïÿœ;pªž?	`ï5ä}?Wüù?Tvì~?Œ?ïô87ê~?Tvì~?Œ?{T4ÖèÏ?|tY»"Ø?ïÉW–ƒ©\?|tY»"Ø?Š¸.È#÷?"ï½M?ï•Dúí?"ï½M>SE0æp>i™x—Ão…?ïÿÿöVM>i™x—Ão…PSR4FGL J1048.2-5832¿š=p"êŽh?â^$ãåFÀ6_c-תÀ:?aÀxi@ýÊE³é@Ñ$šéû²?'[r¹ÓBT?Ò¦‰l$ìI@<"™(Z'@"›NÐrŸ?ï:$n:¿ÍõX‡*¬&¿â5¹ö0s¿åh2^L¥¿ìºr•;f¿î¥¿—°
PSRPSR3FGL J1048.2-5832PSR J1048-5832?p·ˆÒRñà?YÏ­'n?ïސîiŒ?YÏ­'n?¨ Y3Drm?¥Pu³<V=?îuúl‡ª?¥Pu³<V=?‹é–÷Ž?&×#J¯g?ïYù_kº?&×#J¯g>+ÊöY¢E>'5D+ýÚ ?ïÿÿ»GÐ_>'5D+ýÚ ?…a3 ¾¼i?·4ÜB}]?ïª{3}?·4ÜB}]?|þäi§ª?-‹ÇPŽq?ïÆ7¶ù?-‹ÇPŽq?'•¤•ÁµÒ?cƋôL9?ﵩm½Ù?cƋôL9=´8ªö·ÄÐ=óº(Rùjî?ð=óº(RùjîPSR4FGL J1048.6+2340?ì5E½W›@O0¾
í)À:5¸H±JÀ<X•âTô@®°¬Õá@5^³¾?·ïðh]a…?É^KòK@
yT!ÀD(@ª¢€s?ãÛÀÛ|é¿ß‡¢u‹G¿ãwr'dÈ׿âðc	º"å¿ïÿBu?ïƯ²	ÒèPSRPSR3FGL J1048.6+2338PSR J1048+2339?îXÉjö ·?­uÞVì.?ªsiNæ&—?­uÞVì.?ïb#WX5?¢ƺã6?"»•Ý+W?¢ƺã6?íÜ°C˜õÊ?¡!¤ÁE#-?±}âÊ^4?¡!¤ÁE#-?òqïS?CÆÆ{äx?¤ö€ÜP¦Ë?CÆÆ{äx?âŽo¿€ˆü?ÍÆŸgÜ*?Ú㠀þî?ÍÆŸgÜ*?è"®6u³?ÎÞ4¢¸Àë?ÏuGë&)5?ÎÞ4¢¸Àë?ÞäàGä4?À?¿LuhQ?àóÜ
æ?À?¿LuhQ?çYR烇?¶r	´a?ÑMËZ0øñ?¶r	´aMIXED4FGL J1055.7-6028?ïʖYѶ¿çŽ2BrkWÀ8¬À¾¡'À;˜À¤ @SÃvŒÏ@*]Œú?·³%ë!!?ÔÀÎý(µ+@x_»Qz@êǧŽ?èþ2Ö!ª¿ãÒò䏿ÕØǁß=¾¿åÁßԍí¿ì•ªåò8¿äaSlŽž"PSRPSR3FGL J1055.8-6025PSR J1055-6028?"ºmPoÁõ?"Ðåы™?ï­Jç|H?"Ðåы™?Ãä‡ÿhU?ºs>Õ"?ëÞ%ê ?ºs>Õ"?Å¥u'J½?¯P5åyÏ?êºV¢›mQ?¯P5åyÏ?É×õÂ0ß?©L¦î3'^?éºÊsÈ?©L¦î3'^?bů}UÉ?[=žÞ]\?ïí:P¼c§?[=žÞ]\?ˆJµ‡–Ö?ŒwÜf[?ïžÕ*
âÔ?ŒwÜf[?ž«šâ"Á5?–…fJ¦†+?ï
£)ÖÖ?–…fJ¦†+?w¹é`x[?iHo€?ïЌ,ýÊ?iHo€PSR4FGL J1056.9-5852?ís–r<?èîš|îhÀ9×AšÕÀ;Å<¤ËüÃ@?bØè9@ìåÜhKC?Áü	ÂÌn?ïÿæÀ
@"vsBí»?ö–£Þ S¿ïú˜i²?ïþW‰SÑ8¿Ò
è@EÀT¿ì2j€§ZL¿ïÿû-2h2¿ïÿ'¢."'PSRPSR3FGL J1056.7-5853PSR J1057-5851?K6ê ª@ß?`?ì³SËJ?ïù2Enìi?`?ì³SËJ?¯®jÐÈÕ?§9¦R°>0?îRó~#?§9¦R°>0?»w:‰"½?¥õ
ûÓíË?ì'®Íˆ_?¥õ
ûÓíË?P&Déïõ/?8Þ^Ò,?ï÷ìÝRDà?8Þ^Ò,?­™Xӗ"?ËG@ˆ}´Ù?î&jr"ˆ?ËG@ˆ}´Ù?í¤ƒ6'œ?"]7ÌF«e?ï¸ImºÌ"?"]7ÌF«e?˜`"rñ®?£Yø(B?ï<û\hqë?£Yø(B>ãóH)§ã>Ù ˆ	$J?ïÿì¿<R>Ù ˆ	$JPSR4FGL J1057.9-5227¿ïÕwxed@•ÜÆ?À5òtBÇüÀ:ÄëQóÛ@¿àqoXþ?ÿé}£~?†NY²×`Ø?áRqQ{ó–@TM)Ür\>@'Îunl?˪OŸO'
¿¸/g¡¤Õã¿Üà"È×˿钂¹ƒCí¿ï¤ƒ!Ýö@¿ïÿª9ú͑PSRPSR3FGL J1057.9-5227PSR J1057-5226?n7+Íҝÿ?tÒ³n4?ïáÈÔ3:?tÒ³n4? …{Â}š? eézÒ?îÿǨmv? eézÒ?¡w\º¸o•?–GÃ>?îèŠ4À×?–GÃ><-',¤?qG<n},²ó£?ð<n‹˜7‡?]l´àÄV?PÀ#€<˜8?ïñI¦3¨E?PÀ#€<˜8?tÀ½ÿYÂ?}'÷Kùð?ïÖ~ƒàí
?}'÷Kùð?‹?ўâ?ãO—®7)?ï"¹Ae?ãO—®7)?ðPSR4FGL J1102.4+0246?ïü"$(˜@K+J#9ÀìÀ;NVCÙs¤À=Y/F>©@b«@a¼þl'?Ô¬Ù<qËI?ïÿüÉï£@5‡†qž©@'H¿·e‡¿ìäšHì¿ÚØÐ;AI¡¿ÌoDö³¿ìoç¨m¿ïÿþˆ0»Š¿äðŽ¾^:PSRpsrPSR J1102+02?íÄ5H%!'?ºwXHÚÁ?±ÞU¼±1ø?ºwXHÚÁ?í°n¡Í?µÛG¾L?²|Šó)&?µÛG¾L?ëŒ1jõÜ?©O9yù_5?ÃÍÏ:T(?©O9yù_5?éUˆç´s~?°5"É@?Ê©Üa.2?°5"É@?ë쬎¥?ÇQjþø?øOùMÅl?ÇQjþø?ç<=•Y:?Ð
^•ëí?Ð凄ÕM‹?Ð
^•ëí?Ü{r&¸ü`?Â	ÝW<q?áÂF죁Ð?Â	ÝW<q?ÑüO(S¨–?º[R$ ?çØkÖ+µ?º[R$ MIXED4FGL J1104.9-6037?Ö³5¶_ö¿ÚQ¡GãÄ`À8HzÿzŸÀ:Æ:¸b²@áTzU±@õ´'S+÷?²×f®µµ"?ܼñBM@"ëQX¸'ú?øß',꙼?êÃ'ëk¿Ó?¦n£¿ßÌ! Œœ¿å‹¡¿ï¿íBÞô¾¿ïÿÿ)@k*PSRPSR3FGL J1104.9-6036PSR J1105-6037?25¤à¯Ê?/ʞ "óì?ïý½y-úu?/ʞ "óì?¯
̓/?¨×‰8TX"?î&þ5i]?¨×‰8TX"?''Ò	«-?Žp:"jI?ïo.Á*úw?Žp:"jI?m­t²üa{?[×čñÑ?ïâR‹p¿Ž?[×čñÑ?=¯	sOù9?+jiYâ8o?ïüJÃJÔ?+jiYâ8o?öKA¹4?ƒ=⭁?ïÀiFô?ƒ=⭁?'ŸÂŽi"‹?c9jþÓ9‹?﵀ö	²?c9jþÓ9‹>÷C­Í­Æ>ï{™ÌÍf?ïÿÑxqðw>ï{™ÌÍfPSR4FGL J1105.4-6108?¸ï••ý"˜¿ë˜<8dÀ8°8\gßãÀ:â¤itš@È(MQ@eº|h0k?»ÈÉ2
™F?Ôō]¡í@Y:´0ô•?ûÓÒ¥~Õ?ëtž½ÅÈͿӌÎû%OÆ¿ãê™fmó#¿çÔoŽ-TÍ¿ë€<01öó¿ïÿþ½à ¿PSRPSR3FGL J1105.2-6113PSR J1105-6107?•LÀîŠFF?¥WFiÅO?ïU™ø§Ž?¥WFiÅO?»rƒ?»ò?´τ¹Âí?쑯˜Ÿâ?´τ¹Âí?ǂ]?ºS?°
²`ýÖ6?êh°:k?°
²`ýÖ6?¬ãÉ£ ?'˜Z"ðt?î1΃–?'˜Z"ðt?"6ïtÿ?®"ù{lW?ï»íîýƌ?®"ù{lW?"Ï@3oñ?ˆ³çH…8?ï¬Ã›(m?ˆ³çH…8?Šà€˜G³>?|#Åxì?ï"}ýu¥ã?|#Åxì?I,@ÕÀz>?8¨>7¸ŠX?ïù´ï¶[Ç?8¨>7¸ŠXPSR4FGL J1111.8-6039¿Ú©=ó$ó¿¼$(ÿ'½ßÀ7—V¸sytÀ:'o™ëÎñ@ <|k‹iU@ËŲý?§hìÁ?Õgùä]K@*ß¼@ùý‡?åEfîVŠ¿ØÌï,¿Ø>("®zý¿ßw»B¶³Ü¿éêœ÷+°¿í'T·PSRPSR3FGL J1111.9-6038PSR J1111-6039?I:·BŽsƒ?Hè[@ ¾?ïù±R%šL?Hè[@ ¾?¬aTÇ`©?¥&²yå?î9꾿Õ?¥&²yå?Àv0ïó(½?ª­¡ûr9Ÿ?ëâsÄ5Ñ?ª­¡ûr9Ÿ?ZU0¦>'B?RىóÛ?ïòÕg¦‡?RىóÛ?T
KtŸó|?IâÙÛÞ'e?ïõùZ/²†?IâÙÛÞ'e?|¡XÏÓ?Fsv&?ïÇò½Ç?Fsv&?ª¤?œÅjz?¥Iè¨Ô<?îU¼îñ)?¥Iè¨Ô<>×½pŸq+>ܗM}f
?ïÿô!O…ú>ܗM}f
PSR4FGL J1112.1-6108¿ãw/L¿á8­€¬7×À8•nÛí÷À:g µí7@ DØÒ³'@¨^=¢ø¾?ƪ^û'?Ͳ 8¯žê@RÎ-±ê?ñk	Ãù¨¿ê `þG™?ïKÄúpt¿çcÅ×惿ãíNL"-I¿ìTA ´@¿àÀ*ݤ5PSRPSR2FGL J1112.5-6105PSR J1112-6103?Ó·x'&Í?Ñoø»¾¶?æ$wC¶ì™?Ñoø»¾¶?Ät^eÐ?À`×L=×b?êø¢èf ?À`×L=×b?ÞÕ(—_ñ?¶âY•·P¨?à•k´Pv‡?¶âY•·P¨?¸:SSK‰?¢Ù-Zæ‡\?ìøµ•Åñß?¢Ù-Zæ‡\?Å Ôc'í?ÄD"VëÔ?ê·Êç;ÛE?ÄD"VëÔ?‰69ä,ƒÏ?~=3vÈ?ï›'¦G°?~=3vÈ?ÆT~Ðs(?­6s›¸j±?êjàKã5ø?­6s›¸j±?U¦²Ù…ê?LœseÜ î?ïõ,þCoõ?LœseÜ îPSR4FGL J1119.1-6127¿ïúû܄е¿áv"Ž¾À7܉ð¯*%À:ÀY‰QÞ@iœÄò7ë@J<d4]?¨ZàÜò?Å­7Ü_ï@;ÕýÍö˜@È¡Îï?âèˆ6ê?Ôkf€g™l¿ânE1by¿äärp_äl¿éBpˆ(X¿âÕð'3¡mPSRPSR3FGL J1119.1-6127PSR J1119-6127?åh?hR?ÏhýpG€?Õ/ÿ/[É?ÏhýpG€?Ðë£Êþt?Æ­¼òÓá?çŠ.€Åô?Æ­¼òÓá?趨Ÿ,;Ù?°¯Lß+Ê?Í%]ƒO›?°¯Lß+Ê?Ø9¦<È»Ï?³ޓ¥?ãã,ᛢ?³ޓ¥?ĺ©
óŒ?Ëd¹àXgB?êÑU½C9]?Ëd¹àXgB?'Û¾#´¥?™ž·ÀÀè?ïi"â_Ë?™ž·ÀÀè?ߎU§Áu?¾[XZ"úñ?à8Õ,vF?¾[XZ"úñ?—
[
®'ó?†8RE¶Ý;?ïG­'¸M0?†8RE¶Ý;MIXED4FGL J1124.0-3653?Ês	†€Q
@6ÁÁBá&À9#ˆ©[®À<JDÇ°-@óG;¨Í"?þOU!š"?¯Õ?Pç"?ÕÄ C@%dBAÃï®@¿é³¸SÄ?ïÿQŸ/пÊ
Þdú«'¿Ú¸©>Ó$€¿á'Þl	¿íR«ž~Ü¿ïûªÐù'7PSRPSR3FGL J1123.9-3653PSR J1124-3653?YÕXAùŠF?Rf'·P?ïóT¿+?Rf'·P?¾Û)ý¡Î?½‰©ä?ì$ŸzÀKÆ?½‰©ä?¤ò&!͑5?˜Æù;O=S?î°ÝÕh}?˜Æù;O=S?™ªàhàê?‹Ô¦šdï?ï2¨ü¸ø¯?‹Ô¦šdï?gû°«Õ—?b3'xüô?ïèO‰ÄÔ?b3'xüô?œ‰°È~A?œ;¹r/¦?ïk²¢÷^?œ;¹r/¦?ŽºߖQ?"9`(ž¬–?ï‡øôëFW?"9`(ž¬–?;ˆS«+ë?3·Õ‰QÕb?ïüŽõŒð¥?3·Õ‰QÕbPSR4FGL J1124.7-5915¿ï¾–8f"õ?ü;V¸sytÀ7"^±f>ùÀ;ÔoX}p@!õÅ¿g_@_Á}ä1?!§"Kâà?ÎêõVÙ«'@(y!S6ß@-¨ìô-¿Ç®†»›w¿Üf9e&u`¿ä0&8xí¿èöÚQðœ¿ìÄw…¿ä®ÑnòüâPSRPSR3FGL J1124.5-5915PSR J1124-5916?ŠÙp²?'õ½Ô-á‡?œ›Š=?'õ½Ô-á‡?­P¥HŸ?§*¹¼Ý?î/ÿ«,¥6?§*¹¼Ý?Êþym)N?°~H@.Åð?éza¤µ¬?°~H@.Åð?r†ùëž^?d™ô©Ò?ïÚò
	d?d™ô©Ò?pu_\?ɪ?m¨v@£?ïßAZ¾=?m¨v@£?€!JŠ‹1i?'Þ¦Oõµž?ï¿zÕÅU?'Þ¦Oõµž?Ÿ÷¡NÔ*b?–˶Úï'?ïBõÀXm?–˶Úï'>ô=ð$²¶>ð¦üÄlø?ïÿ×á¨Ññ>ð¦üÄløPSR4FGL J1125.6-5825¿î°mJ[@À¥º9LRÀ9׋œ€ÕÀ<T›ñb®@ )c:âÔ÷@CüäŒØ?Àž":ê?᏾ˆfk@­'"ª?÷«]ƒé¯¿Ï"'ª>˜?ǗOýÄ;"¿Êµ_]]©)¿ÚHE¾ûþ¿¿íŒ*¢k¿ïÿ¬óéqHPSRPSR3FGL J1125.3-5824PSR J1125-5825?‹öHÖy©?™övÒ4ä»?ï&ßùái?™övÒ4ä»?¸<$ˆwB?³_ÞUáh?ìø{ná48?³_ÞUáh?¾(…Únj?¥ñ`_N4º?ì:ï\ħ?¥ñ`_N4º?°ë9!Zh?'>Ÿù?íâ˜Û¥úó?'>Ÿù?hš9Ðyá3?bþ°òŠ!?ïçeÆ>¤g?bþ°òŠ!?ƒŸ^]æŸ?†E)2†îz?ﱂ†­ƒ±?†E)2†îz?¥‡Õ†`«?¢{™ê§r?î§''Œ?¢{™ê§r?dÃ. þ~?R!â®®z7?ïë<Ñ…j?R!â®®z7PSR4FGL J1126.4-6011¿í­Ñ\ÝY?îÅ2@QÀ:"ä;~[PÀ<?‰öŽg6@j­b#`­@Êþ§°´?ÑGAˆ
¦?æ²uhaé)@¤X9|ùP?ü÷s¼»1Å¿ïÿcW¾,÷?ïý(IË%-¿âÖ斢nT¿ác¿ø¨óª¿ïÿÙi"A'¿Õ›Ä¡Û¡PSRPSR3FGL J1125.6-6012PSR J1125-6014?íXwj´n?³©'h=z6?µ?lCÎu"?³©'h=z6?àで¬?ÍÆÃò[Ë?Þ8ü±ýú¨?ÍÆÃò[Ë?ëªÒƒ'hš?¥–yßLÔ?ÁTµñ¶]—?¥–yßLÔ?ásÞÏrˆ?²•ª_©?ÝæBaï?²•ª_©?áރáÿí?Êû¦m×7Ï?ÝÎBø<%?Êû¦m×7Ï?°¹OR[i?¼I±J¡u?íèÎUìyC?¼I±J¡u?ä$–§™.?·KÉ
C˜?׶Ұͣó?·KÉ
C˜?ª"1+ÅKf?–êÞ}Õ;?îV¼í(.j?–êÞ}Õ;MIXED4FGL J1135.2-6055?°©Ë p'?Ⱃ`št‹À7Ð*o?RüÀ;4Ôóâ»@'±«^="@+¯EÓHè?¢XèàÞk?Ò<(…a9@&é䒼/Ç@>óp-?Ó3ÊnJ¶¿×M†00It¿áõÖ±R¿æà@è'œ&¿îiΛ&%¿ä±úƒ¿<ÁPSRPSR3FGL J1135.2-6054PSR J1135-6055?c.66o?e>z¾$ý?ïìøѸnò?e>z¾$ý?­l"ÎIH?§´pî&O$?î)>&ΘK?§´pî&O$?³–ºØË·
?¤Ôã(¦3Ó?í(¥Än?¤Ôã(¦3Ó?t-·ÕŽ!I?d3ÿ7yÿ?ïפ(è¾?d3ÿ7yÿ?TYCkü.º?SÞuŧç?ïõÓ^a_A?SÞuŧç?€d¾œæ†®?xè¨ä?ï¾m'åE?xè¨ä?ˆ¼´er¬?x½ƒ<µm?ï
.3;Ž?x½ƒ<µm>ý$oRßï5>õ˜ÚÓSÜü?ïÿÅ·Hšè>õ˜ÚÓSÜüPSR4FGL J1137.6+7527¿ï§²"z"@DeìÃã?À<ÝLvÑÀ=ž™Ó{<·@ ,Õöí@dÀĀÍñ?Õ¨ß<ÿí?æ÷]ßÚ¾@
Dr¦É¢?øçý%	O¿ï–­94?ïÿ—Yοо­dҒŠ¿ßv•¾BÆN¿ïÿ¹‰#)Ñ?·%—"0ÏPSRPSR3FGL J1136.1+7523PSR J1137+7528?í¿#}¢[ú?¹'cæí%?²äí 2?¹'cæí%?ãd­×>?×?Nj²Ä¸×?Ù6¤Qƒ€S?Nj²Ä¸×?êõŽËõ·?¨°—'?Ä)ÇÄÐ)#?¨°—'?Ý7¸^çÓ?°"2¨iƒ?ád#Ќq?°"2¨iƒ?ê5C…T¬ï?Æ*0€%@?Ç*ñê­LC?Æ*0€%@?÷ñ0âÔ?Ã6šÕȍ½?ë³ÇJà?Ã6šÕȍ½?âŽõ€E¾?¿®–"c$?Úâøÿt"?¿®–"c$?¦'øüØ7¢?xi3YÐ?î—Ðp	A6?xi3YÐMIXED4FGL J1142.8+0120¿ì,tÓ´@Mµ\î À9Î{€©Þ‹À<F@îݘÍ@=5?§á?úñўå?¹Å‡Gw8?ՆhD7@P<«ù@ëpTü±—?ߟy'wéñ¿ÒcÀ"?h¿ÒTÑ]Ö¿ßÛAÖNV¿ëêòòÑCT¿è:"DÇPSRPSR3FGL J1142.9+0120PSR J1142+0119?°,=¦4ÏÄ?³1{l'Á-?íúxKb¡W?³1{l'Á-?×âa<8ž?Å¿;×>M?ä@Ïaã±?Å¿;×>M?ÎõþÙS1Å?²G-Ç%¨b?èB€I«3?²G-Ç%¨b?àÛ°<É4?´j_0œgñ?ÞHŸ†m—Þ?´j_0œgñ?‡¥‰
›¤?À¸Nʂ3?ïÂÓàÎs?À¸Nʂ3?±î&Tº?§Æà"	Ø*?íÞ'‰ö}9?§Æà"	Ø*?¨½u¡)Ì?£Œ Í9‹?î"(|²?£Œ Í9‹?´°A"ãnu?¡\À¾Î<?íi÷ÛÌ́?¡\À¾Î<MIXED4FGL J1152.0-6107?ëÈ$W´X?íwƒßóðþÀ95èºiúÀ;£ã³™ @XZÂnO@±æ­j1?¹œ÷rë:?سµÄÈqs@™eéŠs@HÑQkØ?èÎ{·?ïÚ&ò³c¿áªjÂkŸá¿çQ.ƼèS¿ï
¸Á?Èñ:j_kPSRPSR3FGL J1151.8-6108PSR J1151-6108?À­7¹³H?¿‹rœLÝ?ëÔ²"-ø?¿‹rœLÝ?Ğ»
ÿêS?¸à¨á¤å?êØQ<€k?¸à¨á¤å?Ñ~Îôç•r?³†KPÑÍ¿?ç@˜…Œ5G?³†KPÑÍ¿?È
lˤ?§u^¸vŽ?éý{¤Í:—?§u^¸vŽ?pC|û'üè?n¢†‰ÇÂ?ïßyêž?n¢†‰ÇÂ?ˆ.jÀuøì?‰~•§ß'ý?ïŸFU5!Ü?‰~•§ß'ý?™
G2—Í?n‹2€?ï7­Æ¢;T?n‹2€?}¼«'¿b?kùN`ºBÅ?ïĆ©õ(Ù?kùN`ºBÅPSR4FGL J1207.4-5050?ë)B2´'@&՚•BÀ:Ô©: À<€`mþá@M˜f"³@ˆÌ»ÑÓ?¿Úø‰"ò?䂓=_ @E"¼»Ò@»ž`²?ë­2h2?ïÆÖÖ¿Õ^ü· =¿åÜá­¿îXO·Î8¿ïÿ™"{UPSRPSR3FGL J1207.2-5052PSR J1207-5050?š¡"²rR?¦cŒ¶@Ë?ï/Úó£r®?¦cŒ¶@Ë?¼Ò\Èq¸?¸,¿Á­|(?ìe´fñÈý?¸,¿Á­|(?Ŷ׈ùŸz?¬Xfï.i?ê'JÁ˜"?¬Xfï.i?¹ƒE'¦þS?Ÿ> R/¯?ìϗMË 6?Ÿ> R/¯?a3­7£]Ò?r"xÁ­íã?ïîÌR˜B?r"xÁ­íã?Ž¢vs5?'Á-êñfd?ï…v&wãç?'Á-êñfd?˜W/¨å?†4YGÐú?ï=C–Çq?†4YGÐú?sÆ´Z"8ð?bóWÃèÏñ?ïØr—n"~?bóWÃèÏñPSR4FGL J1208.2-6237¿ìž§ ö㪿Ʃ¸J´¯À7ýùp™ÆÀ:'Ӂô@ùx}À?@'í»YÝÂ?°jýNõ±r?Сzäw¹J@ ™íZáÍæ?ÿÏ懳é¿íå`³I?îïV.྿ãäÅø¿ä9€ô¿ì[`®–€à¿ì•†z$PSRPSR3FGL J1208.4-6239PSR J1208-6238?¬§)îô'?À™.'Û+­?î>nÏ'?À™.'Û+­?³~«RÒÖi?«^Ezpz
?í*•³c£?«^Ezpz
?Å·XSJ¢2?¯341vIÒ?ê')ë-Ws?¯341vIÒ?•kÿ¾¢Î³?ƒ"1`WQ?ïT 
éŠ?ƒ"1`WQ?±ž[¥a0Ä?ËEƒµà)Ô?íÌ4‹oVÇ?ËEƒµà)Ô?'B€¾Ži?ƒ@ŽŠü®¡?ï¶õüઔ?ƒ@ŽŠü®¡?ÇLfRGà?"¨Ga‡g:?ïyŜèê¡?"¨Ga‡g:?(_2ßýÈ?!´G*ps?ïþzœ¬°?!´G*psPSR4FGL J1221.4-0634?èËF=¸-•@KÂFŸ¸À9Ûò¿¥œÝÀ<E¿çáü	@îFïÿ@‡ü¹#£?¹_ !·"?ÕîžÄ%ß8@0T9=@dø7^»ø¿Öǁ¿gR¿ÖÌP:ªö¹¿Þ²«£Ý?a¿å{ºÁ1Ž¿îPüD‰¿ÂVjoàb¬PSRPSR3FGL J1221.5-0632PSR J1221-0633?Êå ì"—?Îgdï'?éF¸wÄ÷Z?Îgdï'?ãlì#?Ë+^µdr¾?ÙÑÍ&'Ë»?Ë+^µdr¾?ԙ'£]?´&jœá5?å³ly®uQ?´&jœá5?ê-nÇ?Ó?¦FOŒÞ‰Þ?ÇJD㛳?¦FOŒÞ‰Þ?¡Ç·¢Í?¡',øX,A?îㄅúð?¡',øX,A?º)Ùá:ö?´|–½;ø8?ìºÄÃØ¡0?´|–½;ø8?­ÀL§G?¤ò'ã|?î&.²k?¤ò'ã|?Ëø8<ì+?²ˆNn?éñþpÄõ?²ˆNnMIXED4FGL J1228.0-4853¿ë¶äªRé @+Hˆ/À8ƒ—‰!SÀ;gFvš@ÛýlR@,M€¼S?¦|)`y	?ÉDã^߉@rT¶"¥@<Y¹YÓ[?ï®K75÷3¿æ4€ãÀ.¿âb·O
¿å¢•Ä¿êá,À¨QB¿ïÿ}ß(ïãPSRPSR3FGL J1227.9-4854PSR J1227-4853?ïD¶Ýfð?–O@]|Ø¥?—i$Tõ°?–O@]|Ø¥?èP"[Ûã?È5K
Rà?ν®u?È5K
Rà?ë,m?¬¼á˜ÿÏ?Ãïã›NJ?¬¼á˜ÿÏ?ìÊbìì? ôÖyŸ?¹¬ïPŸ£? ôÖyŸ?ç"Â%î•ä?ÇÔҋd?ÐØ{´"Ô8?ÇÔҋd?Ñf!Á?Ñ-?7g99?çL¸o?r?Ñ-?7g99?æ"x?´Ñc³Ô?Óô×ÝÿÁ?´Ñc³Ô?ÕÛü°j@'?¹×›ÝÁ'°?å§Ê߸?¹×›ÝÁ'°MIXED4FGL J1231.1-1412?ï3¥-˜áÛ@H0!¼jÀ7[ñ˜^À;WÔGëQ@Ú¸æ;é?ù—¡øìx?"äùБ?Ûü}¿sré@G1ïÝëÙ@	÷ï†á>?Ô½C¢—7?š¤^ˆeXŽ¿ÔŒËÀ]RÁ¿ã†€¸!D¿íîˆwÆ¿ïÿÿ&¦³PSRPSR3FGL J1231.2-1411PSR J1231-1411?±T?9ª/?¿²]þÁo)?íÏÕxB
?¿²]þÁo)?·8ˆr)é?º'µÀZ'b?íîñºÂß?º'µÀZ'b?½R׆S?§s­ãád?ìU¼Å5Ÿ?§s­ãád=éŽà:æ>Ábó(Þ?ð>Ábó(Þ?œø–tä? ¼WkxY?ï;LK ÿ? ¼WkxY?— ÿPf0?ŸS4®?ïFø@ğ?ŸS4®?Àí<GÈ°L?°Md8+?ëÄ°î
Óí?°Md8+=$Ø]kG¦Ã=cD(æÑIñ?ð=cD(ö*L9PSR4FGL J1253.3-5816¿—&JA—¤ø@Y˜*ŽÀ:0%™È"À<
9¶Úó@Z¾bѱc@C'ŸÐ€?Ó ¡ ¤%?鍺}¿ÉY@
}œãÐõ@ÀÁ­§n?ëˆGô·M¿·á(V¶E¿éü…%Ä¿êÍñŪ™œ¿ð?ïÿüÉï£PSRpsrPSR J1253-5820?èͺ€Â?Ǭ&ÀW?Ì˽Íüù?Ǭ&ÀW?忽þö?Í-dMm­>?ԁ҄è?Í-dMm­>?êî
*Œ¿?¨ÿfð'"y?ÄG×UÍù?¨ÿfð'"y?çåpñjø?°é¢|xd?Ð5*ü?°é¢|xd?ßn+%a}7?УÞ RÜ?àHêmOAd?УÞ RÜ?©Uš7	'·?¶<:•?îj¦\J®¥?¶<:•?ÝA–5df?¹'X*¡?á_4þåMÍ?¹'X*¡?¶ÃÙ(£Š?©¨¼(8?í'"ÜÑ°??©¨¼(8MIXED4FGL J1301.6+0834¿ïd&}ÀÚ@Q҄ßÎ1QÀ9¨b/ ¼À<[å¯ò¡s@íJÛp~˜?þÚÙÕÉˑ?µ`J~ºW?ÚLó£¦7ã@ ÇTŸ"…^@^¨¯à?ÓÙp^·ÆU¿ÉÉ<Ê`¶Ï¿Ý"€ÐÊÞ¿å£ü~Á&&¿ï
ý˜F³¿ïÿ±[W>«PSRPSR3FGL J1301.6+0832PSR J1301+0833?¡G*åEb?µí4œìr?îëQâ Ê?µí4œìr?Ò°;š?Æ9Rî¿?æ§óbsù³?Æ9Rî¿?Á‡4}Øj?¬'"¸j?ëž²à‰å?¬'"¸j?ÌåÅà'%<?±õ‹ü°¼·?èƎ‡ö6±?±õ‹ü°¼·?ˆ'Kcú¨?¬3ž'Ó»?ïŸbҙP°?¬3ž'Ó»?°tˆvEQz?°½¼k/î?íñnñ`'!?°½¼k/î?¬ô֛̇?¤mªÙVÐ?î0²–Põø?¤mªÙVÐ?†QI_½h?xÃUÖOp>?了ں~Ê?xÃUÖOp>PSR4FGL J1302.4-3258¿äŸ… '/ß@=ØOãm"BÀ9>³"&jÎÀ</#qõâ@¬–"¨q?ú£2ü¬Ž?´ä!s€?áì(¢‹…°@(žZWdjä?ò–"VŽ­¿ÖZE›ÀS¿Ä½¯¸ê¬¿É€Äápó³¿à%°"±"L¿ít0Ôý¿ïþ/{ÎSPSRPSR3FGL J1302.3-3259PSR J1302-3258?^, ôZ?d|^üòž?ïðý±F3–?d|^üòž?À–öâÞ?¼bô£ÍÇk?ëÚ~[ÇH?¼bô£ÍÇk?ª3`S•?š†#Õy?î_¼Î}ç?š†#Õy?^šÀãmù²?Sˆ?ïð²ŸqlK?Sˆ?aiº°tåK?_ҋéÝÈ«?ïî–EH«ã?_ҋéÝÈ«?¡°s¾T?žCt~?°?îïÔùýÚ?žCt~?°?˜Æ_ØV£?˜«`ƒFž?ï9͆û»?˜«`ƒFž>ñ]2×™>ïúá*Ú(p?ïÿÝEjî5>ïúá*Ú(pPSR4FGL J1304.4+1203?ä¼TL»øó@R¨¬1'À;cجëÀ<ñI{t¥@?Ž7£@2[úҙ•?Ï}$"®?ïfAý{k@<o"͊b?üw­ñ•Y¿êÕ>¶I(¿à»J>³‡¿ÁW)‡Óh¿ëìÀ|ÝK¿ïÿ>ñØJ?àæ.¢=PSRpsr3FGL J1304.6+1200PSR J1304+12?Ö2×e#'¤?Ó%´D•±?äæ"Mn6®?Ó%´D•±?×H[Ò2?È?ƒèF>Â?ä[öRy–ç?È?ƒèF>Â?Ùïakn§Â?³MnzŠt^?ãOJH¬?³MnzŠt^?Ñ×h}~B?¶|Ì=âŒó?çKÁ@ôß?¶|Ì=âŒó?ÊtþØkD$?Í%]›xÊ?ébÀIå.÷?Í%]›xÊ?µå¢Í"ì?»>!'ª¡?íCK¦"õb?»>!'ª¡?ìÙãò¿a?¯îÇ‹V5?ëɇP(?¯îÇ‹V5?‹=ngÀX?ƒºK]ˆ?ï"
F*ã?ƒºK]ˆPSR4FGL J1306.8-4035¿Ëi¨ê5@6-gý?[`À9wòŽþ5%À;ܱ?¨Œ|@­•£•ÆÑ@ìgßã*?µÉɍ'Ei?Ãð˜Ä\Ð@¯Ê]†ÃÔ@ZMxß?ï÷¡!MW¢¿á‰Óˆ¨°Ž¿ä{=ï홿ãX)Âq)8¿ïÿø]Ê5™?Ø®'úîôPSRpsr3FGL J1306.8-4031PSR J1306-4035?ïµB^–°¨?†þ*g݉Þ?'¯heR•Ó?†þ*g݉Þ?ïÔq*¥?¦Æñ‡€?Ÿ%q×óAb?¦Æñ‡€?îÝ3%'?•UHùò^?¢,ÎB­I†?•UHùò^?îä‹$-SB?†°'w"‰?¡·M¿¾€á?†°'w"‰?í¿Ü)i¹`?°ƒ{[QE©?²³ÖN?°ƒ{[QE©?èLΒþ'–?Ë÷ ­V‡C?ÎÌÅ´a§?Ë÷ ­V‡C?émrý"ªû?±¤TŽ›»g?ÊJ4uT?±¤TŽ›»g?è^d Å?³ä!8[?ΆmÃ|í?³ä!8[AGN4FGL J1311.7-3430?ïoËgG@<,Š›ÏÔ¿À7…H-–;@À;fDH.lû@̓j5©@X²éÌ·Ô?˜¨yÜ9ý'?É!@ûBV@0 À~á@Ü4ÌesÍ¿›÷ý8`ªÌ¿ÚºìDâ2:¿âp·ù1¿ä²tË•¿ìËLd\ ë¿ëˆG◺FPSRPSR3FGL J1311.8-3430PSR J1311-3430?¡Â|·ê?®Û䌙òS?îãÞØy9Ž?®Û䌙òS?»dH¿aL?º[n-㛤?ì"vèÐ?º[n-㛤?Ո•èVx?¶IÿÐË®?å;µÔ¹D?¶IÿÐË®?WXv}э?UOµÃ›s­?ïôqSÕ?7?UOµÃ›s­?~o³¾Ÿ<»?†V¾mò"?ïà ˜ž>f?†V¾mò"?›ÇšÝ´?œê"OÊò?ï!Ã/{Sï?œê"OÊò?"À)Xòh?·Wáú&9?ëZÏõ©Ãf?·Wáú&9>Êx§&ÖóÏ>ÑúøJêÎ?ïÿùa¢©°>ÑúøJêÎPSR4FGL J1312.7+0050?éž‹6@Oœ1&éxÕÀ8ö6êÀ;øždÚu,@Öþ~ö€$@ŒÏkã}é?®>—?w9G?ßBÚ$ú
s@,mXê|àü@́±ñTA?æêZ±ý=®¿Ã)Ê(ؑQ¿ÚæÝR¿æAP—ÈB¿î釃 U¿ïû	h^ŽPSRPSR3FGL J1312.7+0051PSR J1312+0051?Pšj#[6?QZP|?ï÷²ÊÔ5]?QZP|?ÌG!i ?ÄlzQ$?èî:·¥·ú?ÄlzQ$?­´
jû
H?¢=HŸ{çÊ?î$¿)Bì?¢=HŸ{çÊ?Xd$êà|	?Q¼ÀF?ïóÍí‰/ê?Q¼ÀF?stÏ;»7¼?›Ä]ÓÊáÉ?ïÙa–H?›Ä]ÓÊáÉ?ªãt\ɋ?¦Í²?¡¹J?îQÈ¿Cn·?¦Í²?¡¹J? 5¸Æöî
?¢ËÀ`Â]i?îü¤sgUÐ?¢ËÀ`Â]i>ØHSac)>ݻ̆ä?ù?ïÿóÜ
åú>ݻ̆ä?ùPSR4FGL J1335.0-5656?á?ÝR@­µR\Ä&À9œVwÛÙ°À;ÞIWaç@``LpñÛ?þÊﲪâ—?¿ç¾€-â¼?ÚÓíNL"@^aIÆóo?ù;¬Îª?Ä|*ˆiÆm¿ãUeÂÒx¿ÖT¾\‡¿à£v'id¿í¼<e›:¿ïÿ¶Ï4†PSRpsr3FGL J1335.1-5655PSR J1335-5656?£©¾IAá?±ò;â»?îÅnò0'?±ò;â»?Åöt´5?¼ù'70©ý?깂bùÒó?¼ù'70©ý?Å*öó*ÉF?®JsJ2OÊ?êµBC5M®?®JsJ2OÊ?ؾÊ#?°€‡¶)?ã ¹uøï?°€‡¶)?u'œÕž»?z±:Ì	þc?ïº)õ¥fµ?z±:Ì	þc?ˆ›I'¤¥?‹6>!ñ?Ûöq?‹6>!ñ?¥' ÷'æP?C¤{' ?î¦åð½Ë[?C¤{' ? òáªC?‹í'$R?îðß2ð¬?‹í'$RPSR4FGL J1341.7-6216?ä¯Þ€˜ ?—F~ŽŠÀ8><ÓG:À:$ƒÁÁ@y'w¾'˜@»ÒÄ]''?¿®áÕGšž?½ðÍÝîÞ@'Dé>?ÿŒü?O?ïl™Pž~¿à¼ÃÕ­F¿æsY>	Ðä¿æ0šö奿蛪ëÑtÒ¿ãä"ŸR¹PSRPSRPSR J1341-6220?íPÅÑl*?ÂeÌq¡ò?·ÕyÒ¾y.?ÂeÌq¡ò?ëӍ¿¬äá?Àµk
;?À±ÉLl{?Àµk
;?ä~•»
?·.*ªùha?×áÒԉì?·.*ªùha?ê¥SÈÃÂ|?¨µßÁä>î?Åj°Üðö?¨µßÁä>î?ÛåÃõ¸©?Òê,¯
š
?â
1#«?Òê,¯
š
?Þ¤"<HŽB?Ó®Í#pÙ?à­îáÛ¸ß?Ó®Í#pÙ?ä¡)»w÷?»ÜSÓfÄÛ?Ö½­þ‰?»ÜSÓfÄÛ?͸Nl ?·Œ˜«@g?è'ì~:dø?·Œ˜«@gMIXED4FGL J1350.6-6224¿ÒI½/Ã4¿ÔæÒâÀ7ÞÓMŽFÀ:™c²VÿÁ@[Ë ýQ@EE\*£B?±$Dÿa?ÚyJn¹?@%sçÑ5Z?ýoçáüú?îlT‡@с¿ÑÕ­+ª~¿Ý,iÀc¿ãÛJ^H	Ú¿íã}zV¿ïÿw¿1cPSRPSR3FGL J1350.4-6224PSR J1350-6225?)TyÆÁÎ?$€'®Âú/?ïþj¸Ÿ]?$€'®Âú/?®¯:¦Ö)S?¨C@Öæªd?îU'k?¨C@Öæªd?{˜¥»Tl ?zQ¥z×A?ïÈδiºÀ?zQ¥z×A?`*ðœ…L?Rj©³ïc?ïïÕÝÚ?Rj©³ïc?:õCkž?'«.óp?ïü¡\—Á¹?'«.óp?€³-©v?G¤›LÄ?￝3yv†?G¤›LÄ?'S8˜`?Yd#ìõ?ﶳ¬ÁÈ?Yd#ìõ>å쩈rÊ>Üñ~û?ïÿê./>Üñ~ûPSR4FGL J1356.9-6432¿Ûÿƒ£Ž"Àvò"º7À88É$¡ À:ÿ§Ÿì™ò@eÌ[7ß@?ÛÒú
x?±Ar'?Ö,?Ž‹Hž@çE™›@m¬¯Ëà?Ò àdõ"¿Ù¿v"2á¿ç>	…º¿"¿í*†Pçy ¿ìϦ›àœ¿ßŒ"2T;PSRPSR3FGL J1356.6-6428PSR J1357-6429?´ØÏï©â?»þdÒñÆ?í|DåôLT?»þdÒñÆ?»Ni€³Tè?¶Õ"ÿÛÙ4?ì–2Ïé•c?¶Õ"ÿÛÙ4?ӝJ,Ác?´tL6œ?æ1Zé¹O?´tL6œ?»ü=9º{?ŸÙ‡Q_Çz?ì€xXßȱ?ŸÙ‡Q_Çz?°jÁz?S€?É5‹g§¯?íò§Ðœ˜°?É5‹g§¯?‡'¹5ô·*?‰g×+È~?ï¡õ(-#?‰g×+È~?ºÔ®öow?­§‹6äÊn?ì¥j<2?­§‹6äÊn?UýÚx7e?HQp˜Œ&(?ïõ߬?HQp˜Œ&(PSR4FGL J1400.6-1432?îôÚ`;݄@FˆÚãæÄÆÀ9ɽaõ¾^À<Jã´oÞµ@"{±|9?þèm!kŠ"?»R´¾õ.ý?ÛRËêN½Ó@üC}-RI@zßæ¯÷Õ?¸µÓ9£¿¥TºÂ^3è¿ÙJT¢nªX¿çŠ×^÷\¿ïÿôa¼2¡¿áÎ"7blÝPSRPSR3FGL J1400.5-1437PSR J1400-1431?½'QêŒ?À%ô6ÚBè?ìMÕ®Ÿ?À%ô6ÚBè?ÓæBwìm?Æ2Fa–Ñq?æÞÿÄ	É?Æ2Fa–Ñq?É̇ÜDž?²BÎ6e_?éŒÞΠ?²BÎ6e_?ÛÛÄÕ»?¶Uü—^?âs•"x?¶Uü—^?‡w¦¶î×?¬÷Ã@?ï¢!h¡$?¬÷Ã@?³ePÊÝYC?¸#ì›k£4?í"Uæ͐'?¸#ì›k£4? ±¨Y%
?•š\cãg4?îþ´å5µ€?•š\cãg4?¡4îFù?Ž¯¼iÔå2?îì¾H&à?Ž¯¼iÔå2PSR4FGL J1402.7+1306¿ÅŒÖ+ŠK@Q
Ž`€sXÀ;/´yï°'À=Ag2>@­@Ù0«ï\š@¸/ÿ¢/?Ïn"3¤?ïÿÓT¦J'@j†!퐒@¬ô•=¿¿ïÿÿ>¹ú?ïÿú÷''ý?wäò"䣿çVØ߬޿ïÿüÚ±'Þ?ïÿh@S§PSRpsr3FGL J1403.1+1304PSR J1402+13?Ðåi#@]?Ô«dŒ
?çrKn_Ñ?Ô«dŒ
?ã{äöË_ ?ÍdÆë¦?Ù6iAÁ?ÍdÆë¦?ß,d?´VÍ<ò?à{üñéÍö?´VÍ<ò?ærì=?·_u/=A?ÓÇØx§‡?·_u/=A?ä>1Üq¥?Ô~íĜ°-?׃œGö¶?Ô~íĜ°-?ÁÛ{bBP?Ã15]–n?ë‰!'~/l?Ã15]–n?ØÉÜ£À *?¶é'•Àýÿ?ã›®¯ë?¶é'•Àýÿ?À÷·ìã~?³å6DXÌ?ëÂÿ ?³å6DXÌMIXED4FGL J1411.5-6133¿Ð­™\÷Ž¿Ãƒ'ÓÀ8Žìø¼>àÀ:ZD4"@êýsޟ@1µ"±«?ʔk¿ù?×¥l`¦]ø@"Åyò4e?ô³[,°ã?é­Mî\ê¿ëPƒÀê@{¿å˜fÙS¿ç…NSJ)ð¿ïÿÑ;ÇVk¿åwÜ{~PSRPSR3FGL J1409.7-6132PSR J1410-6132?â£þªjwB?ÕüvUOp?Ú¸«+|?ÕüvUOp?ÅrØœ?¾ã…Blª?ê¾ãx	üÙ?¾ã…Blª?Ýfˆdõ7?¶™²(0?áL»Íÿ…d?¶™²(0?µlVÈí!à? ÿí?íRu&â[Ä? ÿí?Ó{‰Y–°l?Òû> m™?æB;S4§Ê?Òû> m™?Œ4ÇÇz3•?"€¢×?ï,à«r?"€¢×?Îüׇ÷ìÇ?³r¬Ø¬"?è@ÊÎ?³r¬Ø¬"?P"]&…?HRBG€/?ï÷¶€G7?HRBG€/MIXED4FGL J1413.5-6205¿ÊÍÝΧÃS¿çx;»²À6hz™#RÀ:lÞO¬@tðo"7…@ªWÂ^´Á?—ZâàƐ?Ö:[4GZ@9cœ¥½"K?õø‹Âku?ïêF$§5¿Ä:òÚ¨'–¿ÞK9º5ñ¿ã|¯ŒwG¿ëқ
7 (¿îÑ݉¦PSRPSR3FGL J1413.4-6205PSR J1413-6205?XÑwGZj®?m1(æ7?ïó—DˆMÊ?m1(æ7?¨+Š·F™?£æËì÷x?î}G_KPG?£æËì÷x?c¾|Ž,9?‹Â£	L2r?ïŠq
ÇO?‹Â£	L2r>€F.¦@	>ŒÐê–}'_?ïÿÿ¿	âú>ŒÐê–}'_?Cb¥ÚSñ?;•ß¦Ð;?ïû'zå›È?;•ß¦Ð;?}Ëâ*ÒȂ?(§ç®<?ïÄh;lw?(§ç®<?'tó
à?]ñõ"óÊ9?ï¶,3²?]ñõ"óÊ9=—r}§w'=²Ú]ôÑí?ð=²Ú]ôÑíPSR4FGL J1417.6-4403?ŽWcŽü¤Ú@0!æW¸MºÀ9~VG4À;õÐÕp	}@õèä°nG@wCõ"V?·Â<Pg?ÐÒpû•¸@%/ ×{|?üy/ï[íç?ìÃãNïQ\¿ÛÉ#…–,¿áíp¡'Øa¿â"Ànš'¿îà@$Ï¿ïýØ]y­ÁPSRpsr3FGL J1417.5-4402PSR J1417-4402?âípZÓW£?ÉüzÑú«z?Ú%JYPº?ÉüzÑú«z?ÒË\~¨t?ŗÞrUvÄ?æšqQÀ«Æ?ŗÞrUvÄ?ã(¬òÓ`?´*9r§U?Ù®§ÀY??´*9r§U?á¤Ù¹DYÌ?°ÂªZU7Ê?ܶLwLh?°ÂªZU7Ê?šû Øy¿?š—‰'ô
•?ï("ù µ$?š—‰'ô
•?¤ûM"N‡Ã?±A?ó\?î°K-¿š¤?±A?ó\?© ÆPDö?œ¹Q —?îmóšä>Ñ?œ¹Q —?²sÿITef?œ0+ýmç?í±€ÕsS?œ0+ýmçMIXED4FGL J1418.7-6057?å¢#tƒ?À½ªÛ`cmÀ5÷'7ËHhÀ8¾èyÑ@ 
'e¾—@Ât֐›?uHऽ\?Ö]þÛß@6åÖZHŒ?÷¥óýhK?ÒJ»¿à€£ßÓ¿ÒRHù꽿åB
 À>õ¿í]+TB¿ïÿý`éNäPSRPSR3FGL J1418.6-6058PSR J1418-6058?nÖ>§ŽÜs?­H[Ù,?ïá)Áx
‹?­H[Ù,?§½Å·¨Ð?¢rÐ"´ä7?î"/ƒÀS?¢rÐ"´ä7?¤Ð*Ç{M?œÊüU~?î²ý_ß+?œÊüU~>6˛'n/>™^û¦åòk?ïÿÿ~Åô>™^û¦åòk?˜œn÷^º®?Ã*Á^sm?ï;ˆnEz?Ã*Á^sm?{ֆ7Ó³?®¼´°Z(?ïÈRó©Ê?®¼´°Z(?•®t]z""?Œ™ÔîR…=?ïRŒ\ø²?Œ™ÔîR…==Á<(òX§á=õuš¬&è?ð=õuš¬&èPSR4FGL J1420.0-6048?éÜט$F?͈y¡+´9À6­ûmÊÀ8·#24/²@ )Ve'V@üÉï£?³:à?Šj?Ô
›p3o@'^Ÿð˯–@`C¢?Ý?ï©¡ue¿æýôµÖ¿áSS.{=Ž¿æú˜'Bdÿ¿ìC[ªÌ¿ïÿöùŠpPSRPSR3FGL J1420.0-6048PSR J1420-6048?qØƵ†Ú?®<9U×»?ïÜNrSÚs?®<9U×»?®¤ï§Üí?§*Ÿ
ÓµÎ?î±'1.?§*Ÿ
ÓµÎ?ºüjÎnÒ5?©~b@?ì r¦2%¹?©~b@?q	¨óI+?h¾ÎÒùq!?ïÝì®$Ò.?h¾ÎÒùq!?¡$n§Ü?őKeó¾˜?îï=¹Z:o?őKeó¾˜?€Óô#Å?'Øœ=R»Î?ï¼°/»¸?'Øœ=R»Î?®~5AÙ¨Î?¤éZ&[N?î«Ô§?¤éZ&[N>â­´ôځÅ>åo;–Àá†?ïÿíR=Î>åo;–Àá†PSR4FGL J1422.5-6137?éÜùÞ'èý¿äº'J9À7¡77¤²À;
Pø@@ €iڏ-/@Þý'¬?¦¤§tù|?áØì`@2£ôDàÚ¡@l
%É?ë´‹g\?ïӍæÝð¿ÉdxÞ°¿ÚS'Yáæ¿ë‹%nú¿ïÿCý…Ò<PSRPSR3FGL J1422.4-6137PSR J1422-6138?7æÍQX$"?7Z¡wE³?ïý&X·Û?7Z¡wE³?«u£L1[?¥ž«`È@?îH¥Ë" 
?¥ž«`È@?¹åڝ0?§ZƒwKïu?ì܃_à):?§ZƒwKïu>è÷Ùt+>é"QwüøÎ?ïÿçöì'}>é"QwüøÎ?EMy"«qÆ??E[­ðç?ïú¬¡‰'1??E[­ðç?}_¬Ô?€".9_ƒY?ïÅïñ?ö?€".9_ƒY?¡×Û
Hî? ¡›·$Eº?îâ'N¬éá? ¡›·$Eº>G4Î6L¯>ZÚðiš?ïÿÿú+è>ZÚðišPSR4FGL J1429.9-5911?Üä%¸«?ôÜfŒ
ÀÀ6äh8éÀ:'u>p~@£3K[ô@Þ~pHg?˜Öoý'»ö?Ò¦¸¦¥@2PwxÝap@hš6Íq?ÎÐ
YË"¿ØÞ$þÜ¿äOC¿ç£ˆXÿ¿í½ªOÊB¯¿ì¯ÑêBÿYPSRPSR3FGL J1429.8-5910PSR J1429-5911?`í8î'*ò?eÝfؑ#?ïïÇOVÍ?eÝfؑ#?ª¥&-?¥¥ÖÌ|†>?îU®mf4è?¥¥ÖÌ|†>? 72‡?˜˜X÷žú°?îÿ|׎?˜˜X÷žú°?«$jŒÝ?ËâŒâÕ?ïÿ¥SO÷ÿ?ËâŒâÕ?x¼ Ü_¬?­ªè‰¡j?ïΆ¾J¨ñ?­ªè‰¡j?}á"1Úðà?€Í¼‰<¹?ïÄ<÷ÆåF?€Í¼‰<¹?…Ú=Tó?r*m"3ªy?ï«ð—4íü?r*m"3ªy>Td¡‡×e>_Ž-®á?ïÿÿǫ̃î>_Ž-®áPSR4FGL J1431.4-4711?íbS×:'@(§¥	9d¦À9È9¼º0À;ã¥{O+·@x1ü@òR}{Uâ?Àª}—…m=?Ê®ÿ…Ö@%¼Cè@³æ¥;
¿ÙãEó¿Ý)´.pV¿éI-``gõ¿çH~ôÒ¥T¿êˆOúꊿÁë;¢ÃcíPSRPSRPSR J1431-4715?ï©â«ËK?°Ÿˆ°Žß?…‡UúÝJ?°Ÿˆ°Žß?ïÄ©¦"8h?'ok'(S?}«,Ä"<?'ok'(S?ïaÎ èa?‹T	|‰þ?"ÝfBÂ+æ?‹T	|‰þ?ï³,õ›<?gÏc«¥"¢?ƒ 4Á9Y?gÏc«¥"¢?ìNš ]a?¶Ü|5cAÌ?»…‹*ýú?¶Ü|5cAÌ?îY®×R?²@&ÔE¶?ªe'"#?²@&ÔE¶?èŠu³F¥?µÎvbì?ÍÖ)2åk»?µÎvbì?ídB>‹Ms?¡"ž—€?´Ýî‡è?¡"ž—€AGN4FGL J1440.2-5505¿å¿ºž)ª@%4¢žûÙÀ9ì"ì"qÀ;b–ãܳË@´"gÑK@óìÌG?àåîqbBë?Üdrûö*@?,0	³@"K>—ÀQ?ïdG!ý€Ê¿çK;gµÿ¿êLL¿vM¿í¹Ò9?Ö¹õ͔ô¿ïÿþó…õPSRpsrPSR J1439-5501?ï¿_õ;´j?‹ÉŠ~òÄñ?€(ª3­?‹ÉŠ~òÄñ?ïlë¿go·?¡g(ä<åj?'bˆZ;"?¡g(ä<åj?î0Îz)ša?Éø«#º?¬ó[®‹ö?Éø«#º?ïð©¶Ð¿©?R—¿ùüm?^¬'û
e?R—¿ùüm?í CoŒ"?¶'-‡¸?²ýä‰iÜ?¶'-‡¸?ë×äÑâq‹?Ãh¸Ñ_B?À l¸v9Ô?Ãh¸Ñ_B?鸞ғ‹8?¯¢s+?É"µ±Ó!?¯¢s+?ïv2;2þQ?‹³Çö¬Î?'9¸'	/Ý?‹³Çö¬ÎAGN4FGL J1446.6-4701¿Þ%ü­©á@&×W÷7ÚbÀ9¶Ë¢*aÓÀ< #‹öC@úÚý8?ÿq'Ñ8?º'pÉÂ?ۏç¿€Ë@L÷‡‹z@™·
ó³–?ï÷ €=¨¿ãœÀ€
V€¿Ú¢J"
¿å1&s1P¿íˆ}ˆkI¿ïæ¡à×PSRPSR3FGL J1446.6-4701PSR J1446-4701?‰SíĽTw?ëߗL/?HÃÏ^?ëߗL/?×õ›‰D?º?6â\®?ë™®ù?º?6â\®?½1J‹û‡‡?§£q'c?ìYÖ®€?§£q'c?×t_Ô¸á?°Âßú§œ?äEУø?°Âßú§œ?nC"3š'ì?y*Ñí¢u*?ïá¼ÝãÂÕ?y*Ñí¢u*?'"±³G¿?–I¾wåãÌ?ïk߂d§R?–I¾wåãÌ?¨ýë7Lñ–?žò8P?îp!Lo´?žò8P?T±±^~?"üÖ=Ä?ïZrgPœ?"üÖ=ÄPSR4FGL J1459.5-6053¿ê­q™0¤I¿üªØ>À6ÎÿÄpݹÀ:p™ÆC@›h,**@ՙÅ8ƒÕ?–ÝB÷݂ä?ÑsUAûÍì@3fÖE"@«"Ï€0g?ïÇ€\±²¿Ü ïCš3¿ä_Eà´á¿ç—×øyùÁ¿îVÁ"¸Ó¿ðPSRPSR3FGL J1459.4-6053PSR J1459-6053?r‡£V=š±?…ºg8
?ïÚð¹2ˆ‹?…ºg8
?ªà4bÒ?¥Í#û±?îQü¹›äð?¥Í#û±?¾ßoYݟ‹?©¢€HêÉp?ì$ÄL?©¢€HêÉp>îó®àÌ¥>ð,"ÚíÕ?ïÿáR|W>ð,"ÚíÕ?£§¥!a™?Ç-.¦}¹?îŅ¯›¨V?Ç-.¦}¹?{¢«2í–Þ?~ҌJjÎ%?ïȺ©‰¦²?~ҌJjÎ%? ¢Ãû4w?–³aN 5?îõÓÀBù?–³aN 5>=xHÉ­>[§©†î9b?ïÿÿü=íe>[§©†î9bPSR4FGL J1509.4-5850?ì"Ó±~¤¿ã¶¡²lÏ6À6áÐË_ƒÀ:,…'¤Ø'@MÒ±=OA@$³"כ]?žœÁ}t† ?Ø¿Ì^<÷,@3¿â`²È?@¸l"}Ðæ?îrjJ÷u?ёÖ¤¿ÝìWڎ¿ä‰Øá®a¿íW®rn²e¿ïÿÑ ïcÑPSRPSR3FGL J1509.4-5850PSR J1509-5850?Sò8<‰?iÍ?0"?ïöã°$\?iÍ?0"?©øvŠ%&c?¥¢rªF¯?î`x—&³Ú?¥¢rªF¯?'}òyM¬ƒ?'€jÛT?ïtl¼?'€jÛT>ÿÆs·ñ]?…ý"ê?ïÿÀs¼Ô÷?…ý"ê?iS'œ?¥ë{ÏßD×?ïæ¬üf²*?¥ë{ÏßD×?{ÞZ~|¸Ý?~€­§tÒ?ïÈCJØkg?~€­§tÒ?‡Õ–1"o?}8¹Þd‡?ï ©§Èu>?}8¹Þd‡>UÒY¯">vƒ"õôl?ïÿÿõC8>vƒ"õôlPSR4FGL J1513.4-2549?ìïVv@:ö—Oß;À9±WVO˜À<DC;¾òï@ç笳@ÃÝ:ZM?¶ÿ‡_/es?۝}ÿµ,@³Ñà2_@6ˆ*?î˜?ËG¿É£u{S¿àBuüŸ|¿èÊXÿ°J¿êþÈs¡¸¿ïûý<aOPSRPSR3FGL J1513.4-2549PSR J1513-2550? ó`m$±ë?¬zԉ9,?îðÉøö»"?¬zԉ9,?Ì*Ëvœ¥¤?ļÞ1;?èõM"X֗?ļÞ1;?Òz@Š¬
\?²MÜՌ­?æÂߺ©ùR?²MÜՌ­?Ѭ_'O-Ã?®Vpª+?ç)Ð>Øi?®Vpª+?`κ×è'?V–ÍÁ§EM?ïï1Eó)X?V–ÍÁ§EM?©ø<¿³eœ?° ^úâ3ç?î`|4.ö?° ^úâ3ç?žœ¨ô~¸/?"ã6ö«%?ï¸"þ?"ã6ö«%?Œ †r&"?yluj³Ë?ï}ç¿õ×?yluj³ËPSR4FGL J1514.3-4946?·™·@ôfð@<½±¦×À7ëýŽ5¸IÀ;t]ýâŽ@"ÜÅ×?ý;v­‡?¡UÑÿͼG?֖!_K?@1,M‡rO©?ûiùée‰È¿ßNa6ü–¿É‹¶ÂtYC¿Öå+ž{޿ߜjÄÄ낿ìë€K꺿ìÙä!þ£PSRPSR3FGL J1514.2-4947PSR J1514-4946?ZþƖ;9?U'€6l?ïò€œâ=;?U'€6l?«P)úTŽZ?¦Ê"ÐôÖ?îJý`#½[?¦Ê"ÐôÖ?œŸQ|dù?"øð$ñÁ?ït*–¤?"øð$ñÁ?.‰4œÉ'v?._—k$º?ïþl¥'?._—k$º?bYåÞói9?X6™ßڄ'?ïí¦JGç?X6™ßڄ'?Í!Þ°z¶?ƒ€a:µº?ï¸ËxŽÜý?ƒ€a:µº?‹†tIä?†Œ'}?ï"íæ"i?†Œ'}>"¡CªÆ´2>˜[ûŒPã?ïÿÿ[.=Å>˜[ûŒPãPSR4FGL J1521.9-5735¿—L¶^s¿ÚZyMBÔÀ7N#'¬?À:ƒùd@ŸĈ/º@ûbó?£Ó›s
"¼?ÛzA—b@/I¯:ÎÄ?ú0«?ïҟà·ö¿Ñnñ$oöÞ¿â'†ø­%¿èç/N¢¿íázn['n¿ïûÓ {‹PSRPSR3FGL J1521.9-5736PSR J1522-5735?=žYËÕo¼?<ޞ©.	×?ïüL4ó
?<ޞ©.	×?¬ÜßG+k?§֐J.…?î>Â2I?§֐J.…?'0ÆW£ç?r§Ć<?ïvyÌþ(˜?r§Ć<?	'wR!ÀH?³®"©½?ïÿ™¹áù?³®"©½??HÆc%?,![P¯¶ì?ïüçM+­?,![P¯¶ì?€M' "?0?Ã#¼)à?ï¾Éµ§R{?Ã#¼)à?'û¾
׃?^5µ_ÅýÄ?ï´Ëa¤?^5µ_ÅýÄ>g]¿;ga>mTkYñ?ïÿÿè`¯¡>mTkYñPSR4FGL J1528.4-5838¿ÃÓUÊYLo¿ü\¼™yÀ8Î.«6$À;›mµæz@ ¼Êv0^@(éÛÑLŽ?¸Ö—Péý_?äi›Ô×]@#»úëÄ?ÿ#á?¿të…tž?ïIšé$ò(¿Ômc°©€—¿äÀ|A™þC¿í蜁U€¿ïúÖàÌÞëPSRPSR3FGL J1528.3-5836PSR J1528-5838?vѵœ)?°oÇ|ð…?ïÒ]ËÀ»Ð?°oÇ|ð…?±ß«Æ¡6?«,wµ‹k?íÄ
Ÿð‰?«,wµ‹k?'d§Y	?‡]ÌÉu…?ïtßഔ?‡]ÌÉu…?uñSÔZ$?aq}ÿ[֛?ïÔXLêŒ?aq}ÿ[֛?;,)#ð?=ª¿Þ\)?ïüš{Œç?=ª¿Þ\)?€€&€›9Ž?'øÎÂÍì?ï½ÿf@ëq?'øÎÂÍì?ƒxXU¨eQ?bó£¾E&y?ﲞ"B£?bó£¾E&y?Še BÊ?:ùòë¿?ïÿc­ø ?:ùòë¿PSR4FGL J1531.5-5612¿îw…ï²nÁ¿6pÇ¡À]ÁÀ8žo¿«À:‹Á#K^£@")K'ñŒ@E\{+‰?À܃ä{•"?âßøãú@×P +"@½(ûL¿ïûü€¿?ïÿþBe«+¿â@`xÜ¿éÚÔ,<ží¿í…H©¼ýL¿ïÿþBe«+PSRPSRPSR J1531-5610?wožž<?""רŽx*?ïÑ ÂÔa¨?""רŽx*?»»-4ó–?´N—Ä%?숚YnA?´N—Ä%?Ã[8jª˜Å?¯—ûΆÐ?ë)1åUYÏ?¯—ûΆÐ?¹1õeZ=\?¸}X×n?ìÙÁS‹²?¸}X×n?n5|Æõ|T?Žü'b­dÌ?ïáʃO?Žü'b­dÌ?ˆU	Ä:\;?iœÎC?Ù&O?iœÎC? špM'Î?—!·Òî?îþvYëó?—!·Òî?ZO»³V¥o?K:ƒÐ&?ïòØ"?K:ƒÐ&PSR4FGL J1536.4-4948?¸ÅN¯3¶p@%‡CUÀ&À7D¾'wfiÀ;i
	Ó¾@4è-?þXAZ=c8?™t-EÕĐ?Ï¥}'þ®@48ð"aùð@+SÔhx?ïø$B`M¿ÎÒ&þÇp¿ÝÔÜeÇ¿ààÁKdW¿ê7Pþ¿ï-¨§b°PSRPSR3FGL J1536.3-4949PSR J1536-49?ÒOœ	0a?µJ3±²?ÁXá?µJ3±²?©d=ÖË	?¥Ì·Ê¤V÷?îny¼Ôß?¥Ì·Ê¤V÷?Ñʒ¹Rh?°ßpW²Â«?綣{ÖÌ?°ßpW²Â«?ÆfŠì?r#™ÑÎâ?ïÿëR?r#™ÑÎâ?k4[²œ_ž?c±§Aâ?ïäˤ-Ç9?c±§Aâ?|W¼5ñ?€^ëñìq?ïÇP‡¾$?€^ëñìq?¸ê}¶?±¼¦üèû*?ìüb°4¡Ù?±¼¦üèû*>g8¨˜+*>z"†°?…?ïÿÿèê >z"†°?…PSR4FGL J1543.6-5148?×5±¹\=Õ@ù#zX‹²À8À/#ÙùÜÀ;3òuÓÂ@wP»¯C$@C‹«`k?¸ÓfC«Ñ?ÕY:Ë@7Tm?ž|@
jØf¿ãuIX8¦?ï³±=$M½¿ã˜Æ5¿åÃG
H¾¿ïP²4›@¿ïþ)ÉßPSRPSR3FGL J1542.9-5141PSR J1543-5149?
äÝ?™'ܒèz}?ï?—´U÷?™'ܒèz}?ÀxDy?¸"JV2S?ëÿáîá¹]?¸"JV2S?Ǜóuú¡?¯ƒÚË""?ê"¹X?¯ƒÚË""?Δ‹µ!×¹?ªÜøHcŒ?èZÝ·Š?ªÜøHcŒ?nâ§3›òê?'pŒ-k
J?ïáXÍÃå?'pŒ-k
J?‡²ÝAÌï?‡ZªGF"•?ï¡4‹"'?‡ZªGF"•?ˆ»§J,*?yPã¸Å°ƒ?ïb U˜?yPã¸Å°ƒ?žÙX0Á?nT`—è½?ïÀÂN)êÆ?nT`—è½PSR4FGL J1544.0+4939¿é:6ûMa@Izd×ñÀ:ii˜JAÀ<»´Ci@V3Á£xë@üÂ]Þ?¸Œk2ÓçÉ?ÉBÔ+'@ï|i+?ø
ˆ?ü?ë08AíH¿Ë|ÊÌ¿á"lhÞæ«¿ã_j^B«v¿èÈX>/'¿ïY§ÜR{ÎPSRPSR3FGL J1544.0+4938PSR J1544+4937?ïfæ½Óy~?—¸@d#_
?"#(Il:?—¸@d#_
?êJ"âq¨?ü:E®•?ÆÕ¬wö9`?ü:E®•?ï
RTqØq?"_ïȳ	C?žUµp
#í?"_ïȳ	C?èÓÓ*#?«‹6¡Þá?Ïà°³«Wv?«‹6¡Þá?èæK'¿O?Â$q,Ä?ÎfѵÅ?Â$q,Ä?Õ_Ïýóz$?ÏëЦ©«?åPBî?ÏëЦ©«?ê`ÁGÔ?³dßóÆ
ç?Ƕ|ú㜮?³dßóÆ
ç?Ò0ôÈ•?´Á(«è-?æ煛ñô¶?´Á(«è-MIXED4FGL J1553.1+5438¿æ§ËÉËJ@G•ˆ†aÀ:—ù_ÒÎoÀ<Ìò8— C@¼<Vžó?ÿhfx?¾í‡¾‹ý‹?Òó†ŸìÄå@ïÒ¦*¡"?úݹv®³?ハŸ€¹N¿ÑMÓؿރ{Óö¿àïgAÒé¿îgÝÿú÷ƒ¿ïòO]‹KxPSRPSR3FGL J1553.1+5437PSR J1552+5437?æ}›¨´â?Ë3ŒaG?ÓþÈ®–<?Ë3ŒaG?âì~¾vó§?Êy‹°Í¾?Ú'ƒ±?Êy‹°Í¾?æâ)€àn?±wõHm·P?Ò;Û¬þ?$?±wõHm·P?á¦wN§>.?±vü´>?ܳb±ƒ¤?±vü´>?ÊÂêW×Ð?ËÕòÝü?éOEz*
?ËÕòÝü?Ç2<?m˂?ÅÕ»Þ½åÿ?ê3pð$ ?ÅÕ»Þ½åÿ?Í5:Rü•?¶›¿"Z8¦?è²±k{Û?¶›¿"Z8¦?¾ÀEütÁY?¨G‹Ò(#?ì'÷@qgÕ?¨G‹Ò(#MIXED4FGL J1555.7-2908?݃®	W@2€‰ÁµA–À9°^©Ã)À<y)·‰o@¾€+ßVè@x¶Ë?ºˆá~<ò?Ï)U–µd@
\¶â¼y@X=®·8?Õ;Ä|FM¿Ý¢ˆá:˜¿é	ß|Ò¹¿é!YKË°m¿èÒUºc¿ïÿ¨âaßnPSRPSRPSR J1555-2908?îûT›ÒrÃ? ´,Rd¶? J¶C´ºÑ? ´,Rd¶?ítû'&a?´ÄLSHZ?´X!¨Ôòw?´ÄLSHZ?î~˜L#?š'ŒÍìN?¨oşVÔ?š'ŒÍìN?îÈ|
Ë"?"»8n¿"?¯sx?#MÚ?"»8n¿"?æ̏t@ˆu?Æ^šgþI¥?Òfá~ï?Æ^šgþI¥?à$1Ìg‡?҆ºžä¾?ß·œg1ðñ?҆ºžä¾?ä+uæ¥Õ¬?¹AþèäÉ?ש2´T¨?¹AþèäÉ?áŎüú.?»U³ÕsÔ'?ÜtâФ?»U³ÕsÔ'AGN4FGL J1600.9-3054?µZ0LHäè@0o‡z³$…À9¡çÒ␃À<lU\Rç.@!›_íP{?ÿd1m`U«?´£×àýz?ßü©ß7©@"ëØYÈÉ2@Ëuå	"Ž?ï´~÷¬Ê¿´FÕQ€¦.¿ÁÚâ9Eœ¿ÝUÈbÿ¿í]v¾"e¿æßnàˆktPSRPSR3FGL J1600.8-3053PSR J1600-3053?`ˆ£äáj?b^4ý"mí?ïïw\,ü?b^4ý"mí?¼p"ãëÞ?¹JD(—S?ìqû£'"?¹JD(—S?³œÃ\Æ?¡"ÔJ­hÒ?íÌg]m€?¡"ÔJ­hÒ?¬bŠŸçÎ?–÷hçÒ?î?9ך¹³?–÷hçÒ?]$>m_ê?Phæ)X¬?ïñm॔?Phæ)X¬?"N?j? ã´v½í#?ïgoݪâå? ã´v½í#?¡¤©'¬?—ulÚð?îå¿Õm…??—ulÚð?Yà_ó¥êŽ?OóY¸«m?ïóÐ
L"?OóY¸«mPSR4FGL J1614.1-5047?æf­œc?ǵ|N/7üÀ8ãpOô4À:2ðXõ@ ,3¦¹Ú@IèÄzô?ÊÁPlÕ?Ò(}ˆÁÛ@	²|¤–LÞ@:–ê<Ê6¿ï(å!,u?àכ³¿åWiþ÷Ak¿ä(àwúc¿ïÿðÇô ?ïýçAB?–PSRPSR0FGL J1615.6-5049PSR J1614-5048?æܦm"ÔR?ӍûÖ¥"?ÒF³%ºW]?ӍûÖ¥"?ë¨1½<a?Âvݯ¢q?Á_9{ï?Âvݯ¢q?ã½[9Prx?µfn¥>?؅I_?µfn¥>?í≢?¥OžÆ ­—?·§ êi}?¥OžÆ ­—?Ý¿ù-Ó?Ñ´Aʔ}?á }it–?Ñ´Aʔ}?Ú.¶*¶ü?ÔZiuæ•?âè¤ê¹$'?ÔZiuæ•?ØûLý^ºö?·†ËlÌå?ã'YP¢…?·†ËlÌå?Íǀ1¾"ú?ÂÌâf'Q?èŽó[?ÂÌâf'Q0MIXED4FGL J1614.5-2230?æ䧜¼Ž¼@43Ä~I±ûÀ8fé†.ƒÀ;àş±á@ê×™"v?ý™'Í_š?©u}äI?ãMˆÿ˜|
@4f^‰"S?ûq…Þz?ï
–1ÿ?ëP6®è¶7¿Ä9h6¿ãªDâˆõ¿íCçì
õ¿ïÔ»¾²'ÊPSRPSR3FGL J1614.5-2231PSR J1614-2230?\j‹ç
Û?s0BqKh$?ïñ÷J"Û?s0BqKh$?°ì`ð«…G?¯ÍöÓ½t?íâsâʧ?¯ÍöÓ½t?œÉ3{‡©»?•rŸ?ï¶dLþ?•rŸ>ÖÖ¼¼€¦S>ÛC8;u.Ê?ïÿô"¼åú>ÛC8;u.Ê?X·8uIo?SõÃúŠÜþ?ïó¤c»Õó?SõÃúŠÜþ?ŒËÞ3~<?'ïôót?ïŒÐ‡[B`?'ïôót?ˆFä—&¾?})­/›÷‰?ïžälÚ&…?})­/›÷‰>2ûî@ò">E?g·©?ïÿÿýÚ>ƒ>E?g·©PSR4FGL J1615.3-5136?Õ¨ü|׆¿á>Ó°ÜáÀ8Ýñ¸> À:ˆ™|=h@@ *¿;>Åc@¢¡<ü	Ñ?µ°@¥½£?æDí¥Šh¤@&Xn\Ôí-@´€?ï gžÊ°é¿Ô†.B]•¿ÜÜ¥‡äep¿Þ$ò¾#Ñ¿í²
©§-׿ïþÊô<'PSRPSR2FGL J1615.2-5138PSR J1615-5137?$Ðkò-?&¸
ðÿí?ïþ¿¯iå?&¸
ðÿí?®X'"!š?¨Bs;7ÃÏ?îvæç*F?¨Bs;7ÃÏ?"š8&ÂJ?'éÎ6ð‡?ï\.Ð.?'éÎ6ð‡?]³tìN÷?P™9À÷œ¦?ïñ&E¹ó?P™9À÷œ¦?JÈꐣ֍?IûáB1ïX?ïùMÅkë?IûáB1ïX?@Sõ=?ƒct7Aƒ?ïºþ³ú˜ã?ƒct7Aƒ?&aKqý?†êwß]ê?ï‹f{	5´?†êwß]ê>ä±Â™¶+>à‹L_µ£9?ïÿëN(h:>à‹L_µ£9PSR4FGL J1618.7-4633c¿ìÓ'"Ü…@•ê˜+ÛÀ9=#I±À:©ï§Ã(@p{¥<åä@$º¼)?ÛwNëö]À?×» ¿þˆ1@±+ÿbKO?÷°à]"p?á'‡|a¿â8— B•§¿â[eŠ¿a¿ç™è^x±B¿êg‹"ôk¿×$*í"1PSRpsr2FGL J1619.0-4650PSR J1618-4623?íÔ1(fÉ?·Ñ"Üá³]?±^srï;?·Ñ"Üá³]?áÕC¥"?й÷/Õc?ÝàUxµüÚ?й÷/Õc?éHÎ;†¨?°ØÁõËr?ÊÜÇ­å_?°ØÁõËr?ä5YjÌÉê?¸Û,h{°?וM*fl,?¸Û,h{°?âÕG£5W?ÎÊMÛCø?ÛöUp¹•Q?ÎÊMÛCø?°¶®j"?¼ãÏXÿ[Ñ?íé*>Ôm?¼ãÏXÿ[Ñ?މ7<"7?·ÜÊ)ýÆ?à»dsá½ä?·ÜÊ)ýÆ?¡ŠVØXÆ?›ã}µxÍ?îçZ'GÀ´?›ã}µxÍ*MIXED4FGL J1620.7-4927?äP¶3á·s?ÙâûB+»À6ǎö¨hiÀ:hõ2F¤)@ K6r,@i9™m$? Í¤Ážy?áyß¿î˜@7©)þK?üÁ"À?ïK$£Mx¿Ù¨ââ¸Ç¿ÔÔg ÎN¿ÞØ<'g±¿ì>ß¿Ød¿ïº–ÔÃ;TPSRPSR3FGL J1620.8-4928PSR J1620-4927?'ɐ?á¯?+ÞíEœ!?ïþŽC'¿@?+ÞíEœ!?¨®ÈÔ6ý?¤T'[¤ñ…?îudþ ?¤T'[¤ñ…?‹°•5f&@?ŒÇwz?ï'=«ê‡?ŒÇwz>'#œ^šê>›±EáÙ¢?ïÿÿo{‰>›±EáÙ¢?C«Ü'?cN¼ƒ'ñ¬?ïû8û¬Ý?cN¼ƒ'ñ¬?|䗅}ó?ªF¨lƒ~?ïÆ6Ð̋´?ªF¨lƒ~?‡«¼ÿËÛ?€O¾¿ýá4?ï¡Q¾Ø¡?€O¾¿ýá4=Áï÷"ÏIh=Ûaԉ#[i?ð=Ûaԉ#[iPSR4FGL J1623.0-5004?èMÕmk¿Ò©÷þ½áÀ7…J¼Ì¥À:†Œ"ÎX¾@ –üªàéº@Äہ›v?«öÍ&cìä?Ù±y_<{†@%¶å«ÀãŠ@;ùUkí¿ï'½ÂmÎ:?ï|µ«¬¿Ðÿ3ý2›3¿à«;³´M¿éú¿žæàt¿ì^|PSRPSR3FGL J1622.9-5004PSR J1623-5005?Z
€ÅõÂ?d#'	8Ñ?ïòù?ؙE?d#'	8Ñ?¯v2‰°'…?¦¾?¢I™ç?îœ×;»˜?¦¾?¢I™ç?¿Ñ@öÜb?ªFtKŒ-?ì×ÿA$t?ªFtKŒ-?k´wBú—?]åò'OæF?ïäKˆáÝÍ?]åò'OæF?L<H¤%ï?HF|üô.?ïøðíœÞ?HF|üô.?¡<;¸v?9,u—š[?ïÀ½‡µk‡?9,u—š[?¤z"æiq'?¡Ã#b¨
G?î¸V±p-˜?¡Ã#b¨
G>õ1	›î#0>ï¿pS6?ïÿ՝ÖÀ>ï¿pS6PSR4FGL J1623.0-0315¿Ò256ˆ@>«ÅXdE$À9'˜(€QÊÀ<&‹ÿ}#A@IèVk@3/‡­?³xýlÒ¼%?΅÷eҗ½@@,Meä`@±©'×	'?ïô"'òÜ+¿Ýa=@'¿à)Tݧæc¿â\ä¥5¯¿îvSCsó¿ïÿßÿY'íPSRPSR3FGL J1622.9-0312PSR J1622-0315?ÖRôþLÕ?ÇúDnß6?äÖ¹€Ù•?ÇúDnß6?ÞÒ-ß·56?Ïaœ'=†ž?à–é$ee?Ïaœ'=†ž?ä؆DäFÍ?±ÜÊaɯÈ?ÖNóv7rf?±ÜÊaɯÈ?×D"*È3>?°ÇI‡ãÝ?ä]¶j›æa?°ÇI‡ãÝ?‡Ü•÷ái
?…ZŒGßX9?¨ý|?…ZŒGßX9?¹'VŽB}?À¨;ø˜?ìϵ.tý?À¨;ø˜?¿;e/?¯;ÃÄ
×?ìؓ]?¯;ÃÄ
×?§¸¼SÄ?"L[Ð?î"t:ÜÂ0?"L[ÐMIXED4FGL J1624.1-4042?Óð»ª÷¡@©¡N™ÁÀ8P
ýÅÀ;fe€…@w?<ÖÊý@z¼¼´PÕ?©$'bq÷?Û¢‹EC0@)ؽ©CZÉ@8<­…v?ïúeA"_%¿Ñ,}a¡Ì¿à
¯	mg¿æ'"|ú&¢¿ï	OŸz"+¿ïî?CîKPSRPSR3FGL J1624.2-4041PSR J1624-4041?QŽf¥…_?M Ší2Ë?ï÷8̂ؖ?M Ší2Ë?°'é}çÊ?­×0d2á?íîM¢Â"—?­×0d2á? šË±q²?–8ÆRܲ"?îöSED5?–8ÆRܲ"?iåÌôuh?`o2÷ÓÓ~?ïæ32?`o2÷ÓÓ~?Pga¤dí£?nd}ðQ$v?ï÷ÌNïô'?nd}ðQ$v?"õ•*åù?Š}«¸'<º?ï¬)«8í ?Š}«¸'<º?…8û]Ô¨?s"åÿE"c?ï«Q³ž?s"åÿE"c>ð/Y¨.>ïp¯€Ké"?ïÿß߬«ù>ïp¯€Ké"PSR4FGL J1624.3-3952¿Ô@˜»<|@ÃÝ}8ÐÀ9ž3ÆàÀ;ž6`å@'úÇ[ô@üGÿsF?À¾Ëê'Q?Öàþ]ª¨@vì["@æßóÈd?ïý†ì]Œ¿¼vјŽ¸¿Þ5úÀñ¿áË8Bf¬Ý¿ïÿ›‹â ò?ïÞEedÞ§PSRpsr3FGL J1624.2-3957PSR J1624-39?ÍÓ8n'ó1?Åê¬.¥7?è‹1äv4?Åê¬.¥7?ãûb®ÃD?Ï¢öÔL?Øä	:¢yx?Ï¢öÔL?Ù#¯AÌ~?´ -@†×?ãn(_Àñ?´ -@†×?ê¹ý´˜šã?¨ýU£9?Å	-"r?¨ýU£9?§5¥G[?²ãȜÿd+?n±Ë?²ãȜÿd+?©À³€HÛS?·mäQQ@	?îcôÈ$­›?·mäQQ@	?©ÿ»/Æ?š-¨´Þ|I?î`MK'?š-¨´Þ|I?Ë-Ã:Zw?¶õ|ÇMrT?é<41ib?¶õ|ÇMrTMIXED4FGL J1625.1-0020?ξ$ކ³Ž@?Ö9.÷<À8žÎR
À<CN3iº@3ç}R;6?ý}›6QÌ?§™(c)"Â?áE"žæ_›@1â">iƒ?ýð´`Dc\?Ãa}Uì¿Ï§½^DÙÏ¿ÑÆmãv¿ãwlH'·¿ï¿¼¿ïùM^W¤,PSRPSR3FGL J1625.1-0021PSR J1625-0021?S;_ƒÉ{?]Ödn>?ïö~bEœ?]Ödn>?»·r ó"`?ÁSž9ÞÀb?쉻át?ÁSž9ÞÀb?"ãӅ•Ú?vïáÔæ?ï`ácªà?vïáÔæ>ÿ{Þõwë>û®"¶Òµ)?ïÿÁðê}&>û®"¶Òµ)?Kó Qå;?Qªl*O?ïùü9ç?Qªl*O?•àÛ§‡?¤w«*2³?ïPÿZüƒ?¤w«*2³?ŠÏøÊX^?€Þ¶Ÿøú?ï—ÜÀY¿?€Þ¶Ÿøú>gX[ì2æ>nihT%?ïÿÿèê >nihT%PSR4FGL J1627.7+3219¿í,â჊†@EžNaŒâÒÀ:ePÏ%l¡À<»kõò`@1ONFßã?ú¬d\ êÇ?Æn¢ŸýŒ?äv‡*¯@Ì ~$É
?þô¿ÍŠâÈ¿å<ççÛF¿ÛЏ$Äì¿Dr}Ëݹ"¿äج¿f1ã¿ïÿÿ" 5•?ïÿ̾ßú&PSRpsr3FGL J1627.8+3217PSR J1627+3219?¯ªŸ.µ?¼È¤x^¥A?î…V
E?¼È¤x^¥A?Ö¼cX?P?Ë
Ï>
¤%?ä¡ÎSà|Ø?Ë
Ï>
¤%?ÓÊëåÜ?²G°ê×?ævsšŠ
?²G°ê×?×±ð^]"—?¹t´š¦à?ä'ÐÑ5µ?¹t´š¦à?·Fxu·±?ͦW§?í0ñd†½?ͦW§?´ª=°k–r?¶ ĶFÜ/?íj¸JK¢?¶ ĶFÜ/?»âè[ãDw?¨u
rT<`?샢ôƒ—q?¨u
rT<`?¡._ô8Ié?›é4Ü?îí þ'?›é4ÜPSR4FGL J1628.1-3204¿Ó).º•@&ûžŒG¡À9>	 '²À<OB]r¢@ú=ºË˜@_'c3?´S~¾].•?ÞÏ·£Dé@!h0Â?«?ögR]šæ?ïôî<‰¿ÙÕRAì3š¿ÝÂž»¿è˜f~9@é¿îÍê¿&¿ïóêþ'PSRPSR3FGL J1628.0-3203PSR J1628-3205?]sÜ:õ?aWäE?ïñFÃ]?aWäE?¶Ùn]x"ž?´R>ìBì‹?í$Ò4•³Ü?´R>ìBì‹?ªù —U?ä½¯gP?îPmöJ?ä½¯gP?†MqÿŸþ{?qávü ¢?ï¦Ê7ØD¶?qávü ¢?PpÞ¿/«?JMÿþýÀ'?ï÷ǐ‰
ç?JMÿþýÀ'?‹ƒÓGGÞ?"ˆ%k¢ˆ?ï'ð³º_À?"ˆ%k¢ˆ?Šœ\bC¦z?wJèãW‹?Ž'nF?wJèãW‹?#hi°ür?û–<Œ?ïþÉy†(Ï?û–<ŒPSR4FGL J1630.6+3734¿ëª	I@Ešgó
NÀ9ØScTc/À<OÓ7ë)@(¡Ê?©¹?þ"•üV'?¹5Rr=µ?åR›¾aúò@Ì­~«@Oú)ƒ\?ïĬ½bÌ~¿ÖN¾ÿږ9¿ÓÖ¢¤V§¿åˆs¡¸L¿ïÿ÷Ò4Û?ìDÇ_¥'PSRPSR3FGL J1630.2+3733PSR J1630+3734?œÕ¦ìJ?¦¦&Â
@?ïWr‹@n?¦¦&Â
@?щîm}Ô9?Ə'IEï#?ç;ÉAä?Ə'IEï#?»×sfK…Ý?§fR YþÙ?ì…"6D?§fR YþÙ?ºÆVóϘ?£S±÷Â?ì§5!†Í?£S±÷Â?uÞ4˜«å?}ïvÏÍg?ïÕÄCÖx?}ïvÏÍg?³uòh'?¶u"¿…¶?í'A¿E®>?¶u"¿…¶?•È|=åª?‡¥ùƒ¡ü
?ïQ¼:
ÿ?‡¥ùƒ¡ü
?rªÇú`ú?j°ÁjwNâ?ïÚªoøü?j°ÁjwNâPSR4FGL J1634.7+0235?ëOdÆlû@?T›«–òÀ;p>Ȓ«iÀ=8؆>s@I á÷×=?ÿîóhB¹?Ô¡…‹Å›€?ïüÌnØû¯@(™|=h?øš€Y¦‰?´/ȀÈùj?î$¡ÿ?×ÐÇãÙÙ¦¿æµ¹?§4ã¿ïÿý±q&´?ïÉ+ø¬N¨PSRpsrPSR J1634+02?Í.8,lD¢?˒RÑ;Ïí?è´qôäîØ?˒RÑ;Ïí?Ô¤-¸0CÑ?Ìõý |¢?å­é#çÞ?Ìõý |¢?àÞæK4B
?´Ûý¼4Í]?ÞB3i—{æ?´Ûý¼4Í]?Á&§¿"?ªnO<h?ë¶V8úP?ªnO<h?Ãjb"Ÿ´¼?È3‡qk—?ë%gZØÑ?È3‡qk—?°ù0ôD?·A=ŸH˜?íþàܵ^W?·A=ŸH˜?Ò¦T§í?½¢RX›?æ¬Õþq,
?½¢RX›?úÚ.è©U?‡çMZÎ?D][?‡çMZÎMIXED4FGL J1640.1+2222¿ï'Ö!'Õc@C&³÷+EÀ:É[ÇÎ`À<©'¿9@æ!ƒˆ`6@Úmý3œå?ÆR6X¬"s?Ýd)uDP@úÃ")´@¾OhÈì¿¿ª›©ä@?ïóŠ¦·¿Õ­N ¿ã‡ÕÍÛ@¿ïþg¿Víx¿ã_Ř%%SPSRPSRPSR J1640+2224?Îý\S?Ý?ÆI@ˆ'Ï?è@¨þ«0	?ÆI@ˆ'Ï?àCô"$­?͉¾M`¹‡?ßxúÙ¶¦?͉¾M`¹‡?Þ¸.¾H>?¶"@åe"p?ࣱh Ûá?¶"@åe"p?ß܌Î/"'?¬ký˜áR?๘èn¿?¬ký˜áR?ª~'ñ%?¥È.ƒPJÿ?îXÞerî?¥È.ƒPJÿ?öHàÞA?Ãÿæí+ßN?ë_'mÇÈp?Ãÿæí+ßN?¸Ùcމ©0?¥É¶5]D?ìäӄ!j?¥É¶5]D?³µ'MJ?¡CqŠUÉ?í‰\ͶV¿?¡CqŠUÉMIXED4FGL J1641.2+8049?çŽxÝÑÔ@?ij=¯øÀ:Ôcb¥ç†À=f{_ï@ªž+#Å,@O–ü0g§?Â;¶šM?Þj'Ûdj8@°4ß۝J?õ;qE< ?ì?i¢[?î§À&KC¿Ý¡<é?t¿è®JáO»ª¿é¨äÅçÖ>¿ïýªë&PSRPSR3FGL J1642.4+8045PSR J1641+8049?â/¡$ʲ
?Ͷ´'Cd?Û ½¶j›æ?Ͷ´'Cd?׿NÚـ?ÈÍc'}À˜?ä 1X'"@?ÈÍc'}À˜?å\;S?³'¢k¡í?ÕùG‰×YÄ?³'¢k¡í?ÁùRd¯_²?¤Ó¶Tsl?끫fÔ(?¤Ó¶Tsl?²p;YûÒ?°\Ÿ.©ê?í¼ø"À†?°\Ÿ.©ê?·'øýúŽž?»öW=\5?í
Àßûõý?»öW=\5?ÌWy6€MK?´)є'"?èê!²_ì­?´)є'"?"é¶]x?vÏÐo¿	§?ï¬[±4H?vÏÐo¿	§MIXED4FGL J1641.2-5317?ÈòïïÀ?\¯-•À8˳;+À;TÚÌiÐ~@=³é@åŸ+©Ò?³²¹¿î†Ë?Üe;µg@"n½	á*R?ÿn±†uO?ïîºþn/‰¿ÔDûb6¿â¦KÄ#°ß¿éKF¿Ä§¿ïýu@ô¼Ö?ïy§4ƒ?PSRPSR3FGL J1641.5-5319PSR J1641-5317?r¢i:Åèq?xh§¯Â
?ïÚ»-E»ÿ?xh§¯Â
?¼@.®†?·O,,?ì|ú-ê/?·O,,?´c\ÛHÀ?¢"ž-2°?ís"d{¨?¢"ž-2°?³û*Êð-ï?¢HÕyø9?퀚¦x¾ò?¢HÕyø9?ogñì|y?qNïé:ÎS?ïà˜æ3?qNïé:ÎS?¦:üP)*?"´wÐÍá•?ïzÎ'ôCg?"´wÐÍá•?fùjVäR?}c€÷lú?ï|È4"
Ž?}c€÷lú?JåѬEU?Ceºh´?ïù{†U'y?Ceºh´PSR4FGL J1648.4-4611?林g%S!¿éÏ]Àû]YÀ7ÄfUŸnÆÀ:b¸[ü€@ 1)ÆMå@£¢Y[»è?°áà°.†{?Þ9ÚÙ)ý@$ê ¼8*@pjKM[?èY}êçj¿àÌö¡¿Ë¥ô[\6¿áڕwËéx¿ëbšÿË&Ú¿ëDLˊ­nPSRPSR3FGL J1648.3-4611PSR J1648-4611?ƒÝ"°Ò¡r?¯½•Áȸ?ﰉ­	ÛB?¯½•Áȸ?±û•ÙûÇR?ªÎÐï,"T?íÀD²È¦?ªÎÐï,"T?¶ü¾# ?¤¢ÎÈZŒ?í h;ŽÝ?¤¢ÎÈZŒ?~Dš k?otoh@¤Â?ïÃv˟Œ^?otoh@¤Â?±òôð‰§?Ï÷I­Èû‡?íÁ¡nîË?Ï÷I­Èû‡?¼°"Þ®w?'¤¹³`ó?ï¹
?ƒ£Ž?'¤¹³`ó?¡º©»y?˜ðÿa=•^?îäUd,òŸ?˜ðÿa=•^?–6xx5¡?
 ¾4<W?ïÿsNg}N?
 ¾4<WPSR4FGL J1649.8-3010?ï¾¾ì†ÈÔ@"lQ¹07ÖÀ9`òl™†NÀ;ë]"ðÅÐ@I í¶Q@§ºÄŒŒk?¹"ù¼o?ݞPõùl@ ™÷L¿éñ8ŸXËH?ï¢ý$ƒm¿ãÑàd)u¿ÚºûéðÊ¿ã@Bæ.ž¿ïÿþˆ0»Š¿ë·é íö¾PSRpsr3FGL J1649.6-3007PSR J1649-3012?¯.ã{¥U?Éäì[æä.?î
ÈKë?Éäì[æä.?´/…YQÈ"?²…åÐDt¦?ízTÿL?²…åÐDt¦?¿æô´PÜ?§æ–+ãÏ?ì!iuÿ$?§æ–+ãÏ?E1‡¾*õ`?7z3`??ïú³ÚNž?7z3`??ÀÁ[XÚüT?ÓhŽ§?ëÏ©)É@ë?ÓhŽ§?‡³n1)ü?‹»"è›9¡?ï£Ý2~5?‹»"è›9¡?«è´´Ó÷?¡ *~ïúB?îAt´²Ï¡?¡ *~ïúB>אÈeŸ£T>×F,{Â?ïÿô7Ûõ›>×F,{ÂPSR4FGL J1650.3-4600?ìÝÖº}¿î€ž@GmÓÀ7¬r•;fÀ:GÏASC@80Fé@bO̲+?²N×>ã'?ÞÁ»=j@&–V«Þ?¼@RÞ³T*Ð?ÜÇ<? |L?Ë¥ñÁ£ÎÒ¿à4äv]¿å½‹±yŠ0¿îø/¼†-¬¿éœŽ i¬íPSRPSR3FGL J1650.3-4600PSR J1650-4601?\¢¥ƒ Â?q½™œª`]?ïñ®­kÍG?q½™œª`]?°F´

Ü?©¥š¥Oˆ¾?í÷)~m]?©¥š¥Oˆ¾? 7cL3<÷?™Ý"¥å?îü‰Ë<Ì1?™Ý"¥å?W–q-ª^?K"{Hϋ"?ïô4±HÉ?K"{Hϋ"?GG)ÒA¡­?aaXK9?ïú.5X¸?aaXK9?€®&€ºª?ƒdà'VF?ï½Ge¼"¾?ƒdà'VF?†Ž‡èxA3?t[^¯ê'%?ï¥Åà'%<?t[^¯ê'%>Սb
}>ÓP"}ú
Ó?ïÿõ9Ž¨5>ÓP"}ú
ÓPSR4FGL J1653.6-0158¿ãÀâ̓ðª@8ñˆÁÛCÀ8Yˆ1'IÀ;ˆ×§b\@ÕºǬ@‹ôÄü?¤gÉ<õSÕ?Ñí×ßO†P@+ÂÑ(| @Åìäo"?™žõµ5¿ÕÀáÜÿIø¿â£ÿYçÓ¿ç÷Í+—]¿î¢Î–Ñh=¿ïþ'MKã-PSRPSR3FGL J1653.6-0158PSR J1653-0158?f!¾¥Çl<?dÒ>ݨ• ?ïéÞA$ž¬?dÒ>ݨ• ?¶ǧÏo?¸ËmèÉ?í<‡
Üä?¸ËmèÉ?¸Í@е?¦þû1ßØ
?ìíæW¸Mº?¦þû1ßØ
?WÌËÛ@D?O'"'d¼¿?ïô™üb^?O'"'d¼¿?]<oÕ¢tº?M#yZH›±?ïñaÇù±æ?M#yZH›±?¥\wMŠ?–§Ó‡ë¶?jdçz?–§Ó‡ë¶?—éÆ*‡˜?•¤Í¾à-?ï@·é÷ç?•¤Í¾à->ÛrLòb:>Ûf¦>¨t?ïÿòw'né>Ûf¦>¨tPSR4FGL J1658.6-5323¿ÒGm3×jWÀv/¾3¬ÖÀ8¥èYM‰À;š
oTK²@$$5>{@<§…ëfì?®¢Ç{æ;š?àæ
Î&"@)¨U•:@u—†ÄÖ¿Ó¼¢}méè?¨­1žU™¿ãaΆá01¿ê¥)Ô½\¿ïÿ÷fÔJp?¡j£	#PSRPSR3FGL J1658.4-5323PSR J1658-5324?ŽÝߏ_="?—
	"	?Ýÿê?—
	"	?¹	¸ªá(?µØ±£aՙ?ìÞÝ)!›?µØ±£aՙ?¹é'VÏù?¤ oPÅ»?ìÂÏ¿µ&?¤ oPÅ»?'ÆSA¶¥¹?võŽZåo?ï´æ²ã'é?võŽZåo?y6D2P‰?)¾Ú	»?ï͓w§½…?)¾Ú	»?'=¹Ñ?˜pÿ"ëÒ?ïov¸?˜pÿ"ëÒ?™6+<((?=•«±Ö?ï6N¦V@~?=•«±Ö?\­è1±!>ýG9¾‹r?ïÿ¾U#Ú>ýG9¾‹rPSR4FGL J1702.9-4131?äíYý:©?´Ûö5{âÏÀ8t™ŸxÖ«À:=
:{&@vRëŠR)@Æ
c0Q?Ãӑ·øÕ>?á=;•"d@·²ôݍ?þn©›z?£‰£édï?ï ^¿Óêù¿Ý·âYü˘¿ê‰œ*Œñ¿ïÿ§J\D¤?ïïùø?PSRPSRPSR J1702-4128?»Ü}.~îs?ÇcÉ9UR?ì"pZ0"2?ÇcÉ9UR?δõPà©?¼ð¥Hh=p?ëR«ÇÖ?¼ð¥Hh=p?ÒCÅ°+‰ú?´cƒ*Öé?æÞ'ê;?´cƒ*Öé?´hï±?¡_ù-áŒ8?írâ	ÂBý?¡_ù-áŒ8?ÐËÜóò'¿?Ù-)'…nÙ?皆·!?Ù-)'…nÙ?‰ ÷מ5?s²l]Ó?ï™| jŒC?s²l]Ó?®õX òK´?£í՘é¿y?îª}þ™µ?£í՘é¿y?J«¼&ü_?EJEL—w?ïùU2
?EJEL—wPSR4FGL J1705.6-1909¿ïÿþ Y|H@)ý‡ÂÁÀ:7/p0ÄÀ<O!Æ#e`@ÌiiP@;ªe™·Í?α%|fWù?ïþx
Ә™@媴ts?ùùu$dÖ?ïòù¢í]?×S"ÜùÀ¡¿âànrb¿ëå#¿¸è¿ê^ëÈRj¿ïÿYM»PSRPSRPSR J1705-1906?¸Íòäÿí?ƀ—,h$?ìæA£–ü?ƀ—,h$?¾dôÝsI_?ÀëÒ%"#?ì3adQ–Ô?ÀëÒ%"#?ÞÓZÉeº?´;øIØZ,?à–Rõ›M#?´;øIØZ,?aõÁÍ:<?z0oa÷;Â?ï|ðQÈZÞ?z0oa÷;Â?½ôÒqɾG?Ï<iÕS%Ž?ìAe±ÆÈ7?Ï<iÕS%Ž?"yåìzßg?¯|WÕWš?ïd0М)?¯|WÕWš?«;W™ïÖ?«cXx"ÄÖ?ëU1*"?«cXx"ÄÖ?>cŠ'öçã?1å"5څ?ïü3Ž'—†?1å"5څPSR4FGL J1709.7-4429¿é-hGß_À~DÄU/À4h1†:À9qŒ;E‰@&ôî)ô@ÚZæÖc?y5£ •?ÑyQ…XÄè@T8sWæpã@†MZý?¿Q~wÕ$¿Ð›YÂéôü¿ßt†¥ 5€¿ãáû2:寿ë£Q^‹³¿îs'i#°PSRPSR3FGL J1709.7-4429PSR J1709-4429?g`BKn?ì]©†?ï蟽¹Î1?ì]©†?¤U®&QJ?£Ü{º9w?î·*¥+Y[?£Ü{º9w?°ä$ÚL^ ?¤G¯~ù©P?íã{dq»ü?¤G¯~ù©P<+N´Úâ¬<m'Ò'Òڑ?ð<mrAA!?vºJ	R«?­RÎÐzYÍ?ïÓú‹vì?­RÎÐzYÍ?s?fÑ%$?z›­¬áHÿ?ïف2'ïù?z›­¬áHÿ?"|×v[í?rK¡éE:´?ï­ÊËaà?rK¡éE:´?ðPSR4FGL J1713.8+0747¿ì[@Lßt@95Ïþ°t§À9­¯j¼6}À<9HW‡¦R@"»ß@î?ý@YŒcP?·"~ޓ"é?á<ñvu¨@ Áòº`@NJƒ&:§?îpOô4ã?¿'ð]À»¿Ä£Ï½íáÅ¿âí ßôq׿îúS] ;¿ïú­z÷íãPSRPSR3FGL J1714.0+0748PSR J1713+0747?aÿÔN‡à§?i;q±–Ž?ïî+Òt_?i;q±–Ž?»¾4»ò	?»p(­¯ah?ìˆ9¨¿?»p(­¯ah?¤ÇDQ"?–µí
¥}?»4žî?–µí
¥}?¢±dIR?†¹K'ã´@?ïÒêž?†¹K'ã´@?TË"²@\L?V"	Åg±ø?ïõšnß9j?V"	Åg±ø?˜rŸ.ÙÝ,?Ÿ'µù ?ï<kDxç?Ÿ'µù ?‰·|Ò?|?o‰×7g}ñ?ï™#†(3â?o‰×7g}ñ?WÊלb
‡?M?}"dZ?ïô"*ïÃ?M?}"dZPSR4FGL J1714.4-3830¿îã[TÃ~?¾óÙ@£‰2À7_Ÿ¢ÈÀ9¿¬aó:@ –lŠÂ¼(@"=ÚV"L?¬÷ÃhcÛ?Ç1Ubˆ
{@¡\Á¡ö_?ú|ePç¤?ïééªS%¿ÚŒÉÝ.Cà¿áŸ—£ö¿åô¯iå¿é+܂!'Ý¿ç×ó;Ì^éPSRPSR2FGL J1714.5-3829PSR J1714-3830?ºVkFŸ÷'?Ãø¢º:à?ìµ2—,?Ãø¢º:à?·ÎÕ=±&Ù?´/nâÉ©Ñ?í%X ŸÕ?´/nâÉ©Ñ?ÕÊnT,¹-?µœ·Ø1›?åÈÕé£j?µœ·Ø1›?Œ¯!&||¹?{33%8?ïC{f
?{33%8?¨Ç2Š?ÉÄ\øB?îsŽ.EQˆ?ÉÄ\øB?ˆãJº#×ê?"t	À‡¿Þ?ïœrÕ	²0?"t	À‡¿Þ?ÈFàǑ¶?¸GKÑI:/?éîxÇÎ"?¸GKÑI:/?!G'-'?'ͦ
?ïþînÌÖ!?'ͦ
PSR4FGL J1718.2-3825¿ï*c‹•Ÿå¿ÜH%EáÀ7	hQ"1ƒÀ:0«¼²@'ã»-h@ÎåD'×?¦(Öbø¶?ÖÃê¥û¨@-Tšþ§±?ñü^]-'š?ïš ri¿×Ÿ2à§õþ¿ä± Hõ½¿ç+
=²é¿îFY¶T»C¿îNõѨԠPSRPSR3FGL J1718.1-3825PSR J1718-3825?ˆOÐÌŒ&?¯kt5d™e?ïžÀ¼ëz¯?¯kt5d™e?«åÒȈq?¦N8¤å'»?îA¯'ª<)?¦N8¤å'»?ªu±œ•ƒ}?¡	)`	?îX¤æm¡ˆ?¡	)`	>ý·ÛÉ^t>û^\d.<?ïÿЊž¡>û^\d.<?•8HiýÔê?¾'Éþ™?ïV=¼y™?¾'Éþ™?f˅¶Î?'õ+mCˆÂ?ïºdÒ' ?'õ+mCˆÂ?‡ùê"F5?¤Ú"4Fr?ï "c­W?¤Ú"4Fr>Wmʹ'üG>f…\÷Os`?ïÿÿô0WÐ>f…\÷Os`PSR4FGL J1720.8-1937?º¸³æ!¶@#‡ÔCédÀ:!4AP,hÀ;´%ï@zîüÍpŒ@ÏBBš¯C?ÊËúêÂV?¾Ê°'Úb¸?÷â™7t
"@¾P7¥Þ¡?ïü6¢(‰a?Ë^7u¦¿êR®ž8¾¿Û`·õ¥3¿æñX½†]Ó¿ïõ=~æìPSRpsrPSR J1721-1936?ïï–/æ*?eB9ìK÷?`iì÷õM?eB9ìK÷?ïkÙ9d,?¢ÔçE?'"ØÑĬ?¢ÔçE?糧•º3d?ƒÚp²S"?†''s&á?ƒÚp²S"?ïGcå¾Çb?vÑÖ.áò?—ƒH'É?vÑÖ.áò?xeW?ŠyKu"7Ò?ˆaãO>?ŠyKu"7Ò?íÕÐ	Jà?¿úÃU*?·AQ€'ÿ?¿úÃU*?;Ø7(?œPë}µ?¤¥œFÈz?œPë}µ?ìgàƒ&ÕF?£2áa€äÇ?¼ÀûæÉUÒ?£2áa€äÇAGN4FGL J1728.1-1610¿è˜²è¹×@$`;ÄÒ,ˆÀ:S'ŠŸbÀ;ðaXàkæ@³àúVGà@ê%Ðt!?×0y@?å¨Íê>y@/À_A?þ—ÌLÊ3?ØwGà{ˆ?ïôà²\Þþ¿Ä
8èÿ³T¿çÙÁ§Õœ¿ïÿûbâMh?ïÿ<Uñ¤PSRpsrPSR J1727-1609?½¹˜Ÿk5?Àø9¯p'Ý?ìHÌìžy?Àø9¯p'Ý?Àéçq¶*?À#·rÑ~?ëņ#'xµ?À#·rÑ~?Û¤±Òp?³!Éï®Á?â-§röÈ?³!Éï®Á?À†®Á…,?¤ƒTý–?ëÿžTOžµ?¤ƒTý–?¥0îN@™'?ÃY/¸·"?î¬ñög?ÃY/¸·"?‰aj¿k¯3?"êK¢e§?ïšzU9K?"êK¢e§?Ƥ>¹#M?°»L¬ð¨?ê~VðQ·-?°»L¬ð¨?m•µ_!"?`Ó"«?ïâjJn¸?`Ó"«PSR4FGL J1730.5-3352¿äßøVF?°ÎÃG
IÀ7⺎ç¡À9Ú׊•ð˜@j±UXL@½ÀÛ'£?¾»+ÿQC?Ò܌=:ž@<ewS@H)Âq)8?îúæ ³iN¿ã5'»0¿åÞv½÷qç¿éª<P¿ê‡¡8¿ïõ|RÆPSRPSR2FGL J1730.5-3350PSR J1730-3350?ØY—(®¨?Ó0,1{?ãöS4k¨¬?Ó0,1{?ǘ%Cdv?ÁðW©½±¯?êö¯&ý#?ÁðW©½±¯?Ú]ÚPÃè?¶Wòɑ?âóÑמ?¶Wòɑ?ÄßZ_U+?¨¥F5™iô?êÈ)h?jµ?¨¥F5™iô?Âw¿›6Ô?ÒÅY]?ëb8òK?ÒÅY]?"6 êµ"Ë?šQ+mvbù?ïfJøªSÚ?šQ+mvbù?ÁfPÌ¡-ã?®R
Y|¸?ë¦kÌ×´‡?®R
Y|¸?dZÄâàò?]´è9ñ?ïë¥úi×Ï?]´è9ñPSR4FGL J1730.8-2303¿ïî—óÚ¶M@ÇŸ¾vÉÀ9£@4£vÀ;AÜ@W@†ž^ÐDü@(3àØŒ?ÉÓËñÛz?áRíãÉª@;ç)oe@yÙú1ßÌ?ïItR¸3¹?ïÚyޓHÈ¿ä3ÞSÝοë
`z"¿ïþBžHU¿ïøT¥sÂoPSRPSRPSR J1730-2304?Û>43
s†?Ѥ™fß?â`åæyF=?Ѥ™fß?Á4òg³dé?ÁÝOé2š?ë²Ãf&Æ?ÁÝOé2š?â;9Öª5?³¥0…ì¯?Ûó‰ŒR«–?³¥0…ì¯?ºÿcÅC¸ß?¢R¦	ýJg?ì ‡Wˆä?¢R¦	ýJg?±/-Æàð?Ã2®ÿB§?íß*"?Ã2®ÿB§?'µÞöOe	?§ðüý±ô?ïrQ[CH?§ðüý±ô?¸i3Xô˜+?¥±´ñÎ^Ô?ìòٕfº?¥±´ñÎ^Ô?n‹Ô2¿if?d>‰+!Ó?ïát+Ëà¿?d>‰+!ÓMIXED4FGL J1731.7-1850?éüýùs'@ ÂÀð À:;ô¢ÕÀ;ÐÔÚ¸GÛ@öÀ l8@­±™jŸ±?ÎðʐÀW?æ¿Û¢¨‹û@­¢™ó\@(ÿ#·T?ïõ桊(ã¿ââ÷Fÿä6"¡¸!¿íÅWïnb¿î¬ ‡t~¿ïPk®ŒpPSRpsrPSR J1731-1847?àŽš*@ÎÛ?Ò#¹5
?ÞâË«~bJ?Ò#¹5
?Ô¥•PM?ÉéƒM
5?å­@5WÙ8?ÉéƒM
5?èeŸ#Ì?®=Çå?Îiƒs´Ïø?®=Çå?à'wŽè÷·?²dÿ'-v™?ß±â.'?²dÿ'-v™?Ëe§±º!?Ìõ¨"U¯?é&–Ÿ'x?Ìõ¨"U¯?œ}ë«CÂ?²[+sL?ïDٟ¢?²[+sL?ÒeRVÓ»?´&Þã¿?æÍvÖԖ"?´&Þã¿?°ºåÅqW¿?›{5ì¦$û?íè£GmQè?›{5ì¦$ûMIXED4FGL J1732.5-3131¿Ð5°œÑ˜ ?ðã†Lµ»À6ioê›ëÀ:oE	@OÁ^Z@|¢}méè?˜‰:%ë¢?ã/џ‹A@A㦽nŠø?ûȚ$W"?ïáKª"}Ù?Ðxoþ?¶y¿ÑZ³ɹȿãÔÐ=0ã¿î.Ö­ _¿îË¥»PSRPSR3FGL J1732.5-3130PSR J1732-3131?;—ŽÏvÑ?P–,¼FxÒ?ïüŸìÖØ?P–,¼FxÒ?¨QzöÕ?£ïÎjÂÒ´?îzèVɘî?£ïÎjÂÒ´?¡R#åí˜?›¬–Ãȹ?îêÝÁ¼£_?›¬–Ãȹ=ì‡?úxµ9>؁ý@œ'?ð>؁ý@œ'?bªO''! ?'}—Ý?ïíU°ƒ‡?'}—Ý?y+ýtãi`?|•ÆŸrµ?ïͨý{ý?|•ÆŸrµ?Š+Ôøž?‹Ý…£N–?»óî?‹Ý…£N–=œ!8=G™Û)½ñ/?ð=G™Û…ÓþàPSR4FGL J1732.7-5050?è6jÀñªÛÀ"énX£/EÀ9×ò<ÉÀ<2³àl¼Â@·(@7`9%»{?»UJ	c?Ôßs㧄¿@¢;ÿŠ@ôöw5F?ïø€_5ð}?—Ä֚g¿Þ|RáÏ=j¿ã®ŠÂfA}¿ï7iÃèø|¿œ}ãä*ÁPSRPSR3FGL J1732.5-5048PSR J1732-5049?ëŸëìˆåþ?ºŸè=@¨?Á€PMÜh?ºŸè=@¨?îcå$(÷?¯`= }4?¯éÁ±-'?¯`= }4?áÚ3-»
i?´èѤȭÌ?ÜK™¤‰ë.?´èѤȭÌ?í°p»¯?'¤W—ÿV0?²Ì{±"?'¤W—ÿV0?ߊ¯
ïó?Ɔi.JsÊ?à:¨zˆt?Ɔi.JsÊ?⅍oâ"?ÏòÇL*|?Úôå ;ðØ?ÏòÇL*|?×ág¨I¤?·8ú¡\?äuL+Û.?·8ú¡\?áR	óÒS?µ;KM¹ÏÎ?Ý[ýì[Z?µ;KM¹ÏÎMIXED4FGL J1739.4-3015?ïü£ë@?Üã!M»À8¤i×4/À:†ð¬¥åØ@øèë¡@âEõ­–§?Ä_|sp?ä÷—{²(@¿ï|$=Í@nCG'†Ø¿ïЅžºë¤?ïüúz…¿Ù#faˆÜ¿ê@þB:¸
¿í¸^_Ö¿ïÿì´É ÈPSRPSRPSR J1739-3023?Åâw2UV?Γó\®³?ê‡b3jª]?Γó\®³?Áwwe½?¶¤It2ð?ë¢:b&¸?¶¤It2ð?ϖ`/¦Çç?±‡ƒ	OÙ?ègôN?±‡ƒ	OÙ?À™äbj®J?¥M¤e·?ëنçeTn?¥M¤e·?ºª¾ãˆ®˜?΍Yvɋ?쪨#Žê-?΍Yvɋ?‹,Íkí´°?'Búß+_"?ï"LÊOn?'Búß+_"?·0~–ì'¦?´PÖxÖ?íð-=ê‹?´PÖxÖ?gÉh-ˆÃ?Y:òV?ïè6˜Žg?Y:òVPSR4FGL J1740.5+1005¿íPœœû›@4EèÄzôÀ:ý©äjxÀ;ص–Ob>@Ìò"l`Ñ@"à??Æj©V¥ÿ?ÉF…àÕt?ú˜äÓSϋ?ücñ9Æ+?ïýÞ½ç¿åԅ=l3¿ìÊAR¿â&H3uxR¿ïútpe¿ïŽhþÇÜPSRPSRPSR J1740+1000?ïmέ«'?¨ºѯ?'F*B£?¨ºѯ?앲dŸD‡?¼	Å×I?»RlÛÛÈ?¼	Å×I?nq]÷?"Îi7¯¢M?¤9ê ‰?"Îi7¯¢M?ì7ÚÁpçã?BÕn…9}?¾A)ôxÀå?BÕn…9}?íˆÍ"Õdm?³ª,†Tþ?³¹–éTܕ?³ª,†Tþ?Þ]»|ç?ҋƒjÇãÉ?àÑx¢Aø?ҋƒjÇãÉ?é¦df9£m?°'æ")Î?ÉfngrJ?°'æ")Î?×Ñ֛?¶bǿ"<?äv{ò"²?¶bǿ"<MIXED4FGL J1741.4+1354?ï.@3"ý@5«ä›«—À:5òý¸ýãÀ<O)õœÏ¯@å7¿)Ì?ÿ±a‡"à?Á¥[Ä¡Û?Ü	`{ë´@ .s±?þ©l$ìH"¿Í®Ñd65q¿à³xgðª¿Ò3Ðý^*¿åIåý{¿ìË`P¢¯Ã¿ïÿê0ŠâGPSRPSR3FGL J1741.5+1351PSR J1741+1351?ÎKßzW½?ÇÒêY`Ö?èm!j;'?ÇÒêY`Ö?Ñ2»¹ªM?Åí·5b¨?çf¢#*ýZ?Åí·5b¨?ԉpafø2?²	*FZ?å»GÏLƒç?²	*FZ?àœ0'‡?®ÿó'I?ßØǞÜñÕ?®ÿó'I?– ^¶—÷Æ?•˜¼îÁì?ïJý
=Ò?•˜¼îÁì?¤X+LJ`•?¨•"4+©ó?îº}KIg?¨•"4+©ó?¦‰¨g¸a?–U«EM
?î—e~×Bê?–U«EM
?±Ý%¦Öä–?™¦ì¼¡ôk?íÄ[Jî)®?™¦ì¼¡ôkMIXED4FGL J1741.9-2054?ﬤßPš@Ÿ@=ݱ!À6äN¼üÀ:Á±RóÂÛ@%'cœ1¤@)õ>ÛÝâ?š¢x²¼?è
U¾xv3@C¿ohی?þa3™Š€!?íúՉ3ðÈ¿Ì8èê9Å¿âOÅÀi<¿íu!À5¿ïÿ¹žœ¸³¿ïÝ6LJ[PSRPSR3FGL J1741.9-2054PSR J1741-2054?@¦¨={ׁ?^âÇ.Øþ…?ïûÖV«Î?^âÇ.Øþ…?5חüD?¡,¿Âo§?ï~QC‹èM?¡,¿Âo§?¤ãGM÷x«?šùfŸ ‹?î±ËŠéŽ¶?šùfŸ ‹=Ç"àQ‡R™=æ}nòï$s?ð=æ}nòï$s?™Vϼã˜
?Âuùے|3?ï5I'ã@?Âuùے|3?[2 pã>í?x1N±²ÍÅ?ïòf¯Œu?x1N±²ÍÅ?–Óxlá?'3ŒýÝnŽ?ïOYdJWg?'3ŒýÝnŽ<ùÌ&`ǧ=<凧¸@?ð=<å‰ætq¾PSR4FGL J1742.3-3318¿ã¼hÈZ;$¿ûÚà‹ÆrÀ8ÜkÝËùÀ;/:Wꢡ@ŝ7³Ët@tEêPk?Â|˜1º?âú'
‹þ@–¿Ê…Ë?þ=šOw¥¿ê}©Æ˜?
Gç¿×!³ƒûw°¿æhwM>w4¿ímpEã9 ¿ë&€IRPSRPSR2FGL J1742.5-3323PSR J1742-3321?£2xYJL"?³v`MîV}?îÌØz¢Tö?³v`MîV}?ÃK°,®ç?¼™÷fÃd?ë-ôÔ}Æ?¼™÷fÃd?Ã`ŠúorT?«"yY`®?ë'ÝAd#k?«"yY`®?³—ªLgü?—­~U'Î?í
½ÑºÑ?—­~U'Î?tŽ×´Ú?Œ¹I˜VL?ï×ÞãG?Œ¹I˜VL?'¤KÔ]ȅ?™›ñαh?ïjÝ¡†M?™›ñαh?›n¥À'ƒ…?'	)Ž2¢?ï$ŠÒ	*T?'	)Ž2¢?`¶úÃú?P³@v+Ë?ïïIyÞá?P³@v+ËPSR4FGL J1744.0-7618¿ïpñ"_üÀ6t¾ÆyÌuÀ8¦-vZÐ0À<óý">6@˜rÆñìl?ü̲{ï?¨4_>e&²?ã8MžïCð@3Ö}sÉ?ü'@³½?í¸Á>#Q?ÔY3wü'¿ÕfŸÜ©¹¢¿åü­_I<¿ï¡±Ë¿†"¿ïüûÔ!TäPSRPSR3FGL J1744.1-7619PSR J1744-7619?wmýïA?¤ÙK‡Ô$?ïÑ%ݒËR?¤ÙK‡Ô$?¿w½7Î¥?»4ÉÀüÏ?ìY†+?»4ÉÀüÏ?œ˜îñ1R€?"oz²åì?ï8ˆ1½<?"oz²åì>õwŽø·×õ>úÐ$Ë:?ïÿÕ¤N:>úÐ$Ë:?zsR[b>s?šŽrç+²[?ïË[AÃ?šŽrç+²[?¢£cŠÓ}ø?¤‰Î¢W?îÕÉÇE	±?¤‰Î¢W?†â­zEB4?r¸{éþ´m?ï¤uIûn?r¸{éþ´m>S¹e‰ðò>bzK>©â?ïÿÿöVM>bzK>©âPSR4FGL J1744.4-1135¿ãR,þ:Øï@"]·k;¸=À8r¥®À;T¨ŸÆÚE@¾õɛ?@õ\Rç-¡?§G3¾/?䦏ãW@3áœàu÷@蕫"ƒ?ïþ™côÏ¿·üæÅò=¿à-1üÒN¿êꛟƒ=¿ï×ßÖjÛ¿ï÷ß4®]vPSRPSR3FGL J1744.5-1133PSR J1744-1134?HéîÎÊ*X?LØSxoc8?ïùń6¹ƒ?LØSxoc8?˜º»'ki?¡Þ%iåڌ?ï:*#Ñ&µ?¡Þ%iåڌ?–CÊL+ç?{"êƁ?ïMá¯TcQ?{"êƁ>ÑoP‰Ms¾>ÓÚ-Ò,¥F?ïÿ÷H:E:>ÓÚ-Ò,¥F?U'‹Ö©ï¤?Så":J]?ïõ7:1‡À?Så":J]?p-Lp‹Î?'hYñ?ïߥŪw@?'hYñ?†hÌduŠ?u!Kßy?ï¦\Î70?u!Kßy>#e)_oŠë>0zï…Bˆ†?ïÿÿþíA>0zï…Bˆ†PSR4FGL J1745.5+1017¿îs^V¢y@3>­-ËfÀ9šVÿÁßÀ< W¯ê=÷@VWwá
!?ÿFôæÇIÖ?¹=uai|?àE=V¢¤@ 'ÛçòÃ?ùð:æ?â'!,öX¿ÜX°»t4ۿӍÈhûí¿âä
k"ÌÑ¿ïÉûa4Î>¿ïÿH˒:PSRPSR3FGL J1745.5+1017PSR J1745+1017?pGÙ_6¯/?‰Çù™Ø…r?ïßpMx?‰Çù™Ø…r?²MkS"8>?´âi°âzM?í¶R•ºˆ?´âi°âzM?¨"}S@?˜‰Z'
©?î×·?$Œ?˜‰Z'
©?"þ4¶±{?{bsÙfÇ3?ï`ZX2"?{bsÙfÇ3?`W‹â¶Àß?nÁ¤÷Wý"?ïï¨tRã'?nÁ¤÷Wý"?Ý ¦öp×?–¢a)À·£?ïyúÈLy?–¢a)À·£?Œ×Ò³m_'?xìâ
2?µÍ¢?xìâ
2?C➬áŒ?7;€R®u4?ïûXl†D?7;€R®u4PSR4FGL J1746.8-3239?×öb›3UKÀY1¢9{LÀ7Ãu"*ÐÀ:ïoɼw@M,…šT@o<¥¢¼?°süPH?àÿ»lR8²@0¾ß¤@?÷ ÌäIÁ?ïë)yv
£?è)8Þm߿ݸõ_='S¿æ°ô>«·S¿îw.4Ʊ*¿ëˆª"¼àÆPSRPSR3FGL J1746.8-3240PSR J1746-3239?"*€¤X¤?¹àÀhž!?ïf«ú³ÿ?¹àÀhž!?¬?­c&Ë.?¦R©Øòn?î<)é-?¦R©Øòn?®ì."+?£éöõ²w¡?îÁ=;c?£éöõ²w¡>ó¤P
i>ñpÁRxÿ?ïÿØ·U†>ñpÁRxÿ?¡ÜÎâ ¨?º©K=k€?îâ3ï??º©K=k€?~åÊT¹t?'¤ÛÍ^ت?ïÂ4kJ.€?'¤ÛÍ^ت?¢lñù_°r?¬'ù½öº?îÙ0àjù?¬'ù½öº>S›¥ë:ü>bC|i
L?ïÿÿöVM>bC|i
LPSR4FGL J1747.2-2957?Ù
ŒbÄú¿ë
ßòC~ÛÀ6'Ôº××ÃÀ9½åëoO@ÚÙÇ1@Åûø3ƒ?¤RRá#q?Ø^TùM@0yJ€à@eݶ•?çS¼_í%ˆ¿Ô¼"E$Lf¿äjšêÒq¿è'kí"¿îCƒbu–¿ìùÍ¡^	 PSRPSR3FGL J1747.2-2958PSR J1747-2958?°37ñc#?¼4i˜cÓS?íù™ª`M?¼4i˜cÓS?¬o %©!?¦{,ñžs?î9.B]ž?¦{,ñžs?¸ìâ6@ƒÔ?¦Ìɔ*'F?ìâc¸ó7V?¦Ìɔ*'F? ¶ý™a4½?Iľlâ?ïþôå¾?Iľlâ?¿›gÿ1'¹?ÒÉ5Ï«à?ì"Í©?ÒÉ5Ï«à?K<£!=J?'ß›«Ÿ…?ïºÓ
Œ8;?'ß›«Ÿ…?¹þ䢛[?²še¾U"¸?ìÀ#k¿ì•?²še¾U"¸>téyE3>"ÚV'Car?ïÿÿÖÂú>"ÚV'CarPSR4FGL J1747.7-4037¿¶Û,™¸Ž¬À¥P"WBÝÀ9"A!"µÀ;ϜÈù¶@,ØCxz»@ŠwTË?´–Õ™úèi?ܘÞ]ÃՂ@"'6¬dwy?ÿü¨G1lß?ïÉ%x_.¿Ûz1¿•¬¥¿ãFÓ#(#¿æ£»-h¿íœ=þ"Ci¿ïüe¬,CUPSRPSR3FGL J1747.6-4037PSR J1747-4036?b3eœ_Ç?bhl5fI?ïío̎?bhl5fI?ÀٛÁ€Ø?¾›…AÂK?ëəŸÉù?¾›…AÂK?·gŠÑÉÖ?¤~˜
»©?í®!C¥?¤~˜
»©?¡<7åZÉ`?‹ŒÝ	
3Ã?îì<ïš?‹ŒÝ	
3Ã?aæ<>.?lÓà9Â?ïî€ù割?lÓà9Â? Ã¡ò+÷˜?¦iªðWa(?îóÅá{Ö?¦iªðWa(?–ž0P– ?Žk'ß»óÔ?ïKv¦¶Ÿ?Žk'ß»óÔ?;<11eâ?/ÖrçRº¸?ïü˜yÞé/?/ÖrçRº¸PSR4FGL J1757.9-2419?㏚µ"Œ¿˜K?™s-À8xh¶¢¾ÜÀ9ø#CÑæè@ 4ÇÞ%²@«¨?ùA7Ì¿a?ɳ‡i!,@S™ V¸@d¡¼'ãõ¿¶ÍgÑöW?í»
bY'l¿çæ a3÷¿ê^˜q{m_¿é*qš!¿Ð1Ácb%PSRPSRPSR J1757-2421?â«þÊå…Å?×eQ&ý߃?Ú¨j4ôv?×eQ&ý߃?åò4?Ñ.WNÎøª?Ô÷Ãזæ?Ñ.WNÎøª?áàù–Æ3?¸y=ì1M?Ü>
öÒsš?¸y=ì1M?ꉏ¶@ï?µi`.e"n?ÇõÙÁ&üC?µi`.e"n?Ûkížÿ_?ÕÔ<Îùˆÿ?âJ	0€Pr?ÕÔ<Îùˆÿ?È"¡¦ƒb?Ð{n¼²^ž?é÷x—–_(?Ð{n¼²^ž?Þd¹ÝB!?µøS+Èý?àÍ·£^ï?µøS+Èý?¼ZÈ´ lX?·úÆ1›?ìt¦ékòu?·úÆ1›MIXED4FGL J1801.2-2450?áŒõ±Èdˆ¿íÔPXÝèÀ82ÿݛQ*À:šÂn¤ù@=öÔ{@B­Yiþ¡?µÚÎ~cïO?ÎÄ»Ü9§A@>¢Òþ??õåC¼s?íÈDÝ¢x¿ßÆ:ÂÇ;¿áõDD¿ä¿T_™¿é…¡—û¿ïÿ&PÌ¡.PSRPSRPSR J1801-2451?¨¢<ýͦ?·ºK²ü"?îÛù)f?·ºK²ü"?±3ŠÄÈ$$?¹õŸ
êC?íَ§«³«?¹õŸ
êC?ג€½¢î?µùÕÊÞqK?ä6¿¡.þ	?µùÕÊÞqK?•ôör†²?~°Q:ˆþž?ïP_`Z*:?~°Q:ˆþž?d%ò€'É?bi
9–P?ïëÚ
t%?bi
9–P?xé›9,?ŒG"7`ܒ?ïÎ,ÉÀ0?ŒG"7`ܒ?¹@8åÕ?¬Ÿ;ø‡C^?ì×øã3Ê?¬Ÿ;ø‡C^?:!<¤?* žð‡?ïü»Ø2Üv?* žð‡PSR4FGL J1801.6-1418¿ÖðW'Ñw¤@Äk¬÷DpÀ9ß%"åÀ;ÕWµÉ{@Ə§þ6Q@3ƒB??±?Лl¢À‰È?ä›@ãŸø@kf¶~¢@_s"\³?íYiþ¡[/¿¾ò\=îx¿ê5ŽøU瓿î],áŠt
¿»ÂÚô¿ïÿðÇô PSRpsrPSR J1801-1417?é¨êáFÃ?Åüßޑ44?É\Tzç¸ó?Åüßޑ44?ׯѕçç?Д›¾¶?ä(s5
?Д›¾¶?éªú°hpµ?¯< 
Ë*Î?ÉT>^=+?¯< 
Ë*Î?éüCjìe¢?´Ø¯Ÿ ‰f?ÈòTNix?´Ø¯Ÿ ‰f?ÝFs‰\*?Ò³
f£?á\Æ;Qÿk?Ò³
f£?•"Õ»~ˆ×?¥)ŒÜÀâh?ïSÙR[y?¥)ŒÜÀâh?â"h¼ÏK$?ºLHçV?Ú÷.†ai¹?ºLHçV?Àè¶o4¸'?À"à.ÔSÕ?ëÅÒd2ÑÜ?À"à.ÔSÕMIXED4FGL J1802.8-4719?ïÿîÀ^øÀ(qûÅޜÀ:šÉÓIÀ<2w¬ßÇ{@ÃßóE1@@˜ü»§á?Оˆ@Ö´Ø?â9Ž—@§ôÛߏG@؟ÎçÚ?ïy ÕÍýN?ϳù—02οâ¡sîeô¿éÅ# ™5¿íŽÁ.32¿ïþ"ÐÜýPSRpsrPSR J1802-47?í©(¬,Õ\?¾¦ÖÙkÎ?²¶ºŸã/œ?¾¦ÖÙkÎ?ëtÐÙ:³?¼^êy¹ˆ?Â,¼›3ˆ?¼^êy¹ˆ?ì¯c"Ó©?£Pâ?¬'?º"ãƒabµ?£Pâ?¬'?êÄ©EfÅ?¢k†Zýœ?ÄíZêdëÆ?¢k†Zýœ?èO'°?ǽó¶E¡Ë?Ï¡ŠÃ¹B?ǽó¶E¡Ë?ÙéŠ"Žµ?ЧäPè?ãvº¶8¥?ЧäPè?Ù¶˜Ìü?"GhR?ã~$þ3™'?"GhR?Ìèó8¥?°ÿŒë‡ä@?èÅÜ8ƒ1×?°ÿŒë‡ä@MIXED4FGL J1803.1-2148¿Òzª©iùÌ?Éx.û@'¸À7"èG|–TÀ:´v"±Ó@çûZ(ë\@µô^N?¦X"Ãs³?ÑÑ	\õúC@%DæŠ
5@½í;WD
?ì­nB}Óë?îè* dú¿à;­àÎaw¿ãˆP›ùÆ*¿ë˜K$Á€¿ëõe<š»PSRPSR3FGL J1803.1-2147PSR J1803-2149?"{àK.Ò{?±ÅH¦z?ïd ýëAœ?±ÅH¦z?ŸgH'þÀq?¨7¯û
†?ïÅ»Fέ?¨7¯û
†?±–,ôø?£jè<{³?íÞ
:a`ÿ?£jè<{³?Q'£pn?Bèá«ôƒò?ï÷6ý1y?Bèá«ôƒò?pJß':}?¦
¯8?Ì?ïßjAÎg¾?¦
¯8?Ì?g÷uPݾ?u*ä‡ ?ïèè[ôs?u*ä‡ ?…™¯'›?s‡å†¾àÐ?者õ
ûÔ?s‡å†¾àÐ>áFõó~0>Û¦¤'þo4?ïÿî¹Aæ»>Û¦¤'þo4PSR4FGL J1803.2+1402¿ì%!†@)@0êkƒÙ^À:˜û܄еÀ<[›]@@Ìxé÷@Ò¶»éOº?Çâ·ðœ¶?ۘjû .@Eâb`Gh?ö±Ûø8áH¿àfç?¿³Š?tÈT0󁱿á¼v¾MX#¿äHb°Ï@¿ï²äXڌ©?ã÷äþqàmPSRpsrPSR J1803+1358?àkƘçSG?˱ìs4?ß(rÎ1Yr?˱ìs4?Ô½)/"n?Ɍ-¤—¾<?å¡kh6}É?Ɍ-¤—¾<?ç4ŠA¥Ý?²
¶)µv?іë}Ö´F?²
¶)µv?ãÓº8ç?±)"ܝ#?ØX‹ô1ô?±)"ܝ#?ÊÜ°žÝ•?ɑÙh³êö?éHÓØHš½?ɑÙh³êö?£lÇÁ"¡?°6ëIpª?îÇé3hjÖ?°6ëIpª?ƅÂóÁ>Š?¶àæsÊÚ?ê^C°]?¶àæsÊÚ?¯ºÊj®¹?è9SM§?îSYCh5?è9SM§MIXED4FGL J1805.6+0615¿ÖÂÓº&×Û@*΅3±À9öÝpˆÿÀ<1#|
Ü@Þ~Û¨1ã@"à¤ðæ?Áw'iP{˜?à"<›<@#VSÉ«°@ßT¼oÝ^?ïâp"&ñ[?ÀÏÅ0¡¿Óª;½ÆI¦¿à눯fŠy¿ïÿ©-‹S†¿í£?O¦†PSRPSR3FGL J1805.9+0614PSR J1805+0615?¥­£ýû·Õ?µ(‰<þXÎ?î¥%¿éJÃ?µ(‰<þXÎ?¾e…«P%\?»›C<ë™?ì3OJ•ûT?»›C<ë™?Ç(SƦ˜?¬B½!°•?ê5ëVYÿ?¬B½!°•?ÊõYJ–s—?¦–Áîy·?éB©­Zc?¦–Áîy·?¶qȧ÷?ˇþDF´?í?ßq¯±?ˇþDF´?"d£)ôÿ?œç\)É?ïdÚèë¨?œç\)É?˜	P
ÚN–?†•q¦<h‡?ï?µ©-‹?†•q¦<h‡?•"´sÿE	?ƒæ…%M?ïSÚ\M¨?ƒæ…%MPSR4FGL J1807.1+2822¿Ëú†'vç@5‡,ƒì‰+À:£àyQûÀ<2È b@4÷â¥&@á'©?͵ûåi%Þ?Ê®¢jM¦§?ú†¦\ö{?ó™–dïï?âqíþ ¯c?íØ涂޿é8h\	ì¿ë(0Àè#¿Ç°I‰`çK¿ïÿb¶®}VPSRpsrPSR J1806+2819?ïìÞ®)Q;?q¨ƒ"ÓúG?c!Q²òÕy?q¨ƒ"ÓúG?ìÝ9›F?Á%ˆ:K«O?¼3%ÏÑ?Á%ˆ:K«O?ïSaàUüÈ?Šñ —^G?•"Ãõ@g?Šñ —^G?îCShv¥¾?—÷Æn»~Ú?«ÊÉx•¤(?—÷Æn»~Ú?ïÃ˳aÁ?‡5א:ÄN?~&\Œ#4?‡5א:ÄN?×IŽÿ·°±?Ѷááåk]?ä[8€$'¨?Ѷááåk]?íªéV? ¶5
ÀŒ?±ïðçT? ¶5
ÀŒ?áôÇnǒ?Å ÅÊqu0?ÜÄq"pÝ?Å ÅÊqu0MIXED4FGL J1809.8-2332?ܖeâÝÛ=¿ÿóÔ
2îjÀ5˜µnvÀ9²æ[L@ÔQÞÄñâ@ܕà•×?½ÅüV±?ÕÕØ#ÂýÁ@F-¯ ê[S@''[²ƒJ?ç´4ºò¯µ¿Ïñ¤ƒ³ÿ¿àÞ°z¿äé^¾Q^í¿ì¶óé	¿íI³bmˆoPSRPSR3FGL J1809.8-2332PSR J1809-2332?CzO‡E™›?`՞õ§v?ïû!kàxÑ?`՞õ§v?†þ…Z?¡›yØ.
ò?ï‰ä‰½ë?¡›yØ.
ò?‰'–ØÙ|\?ŠÃÞúg]ß?¤s^¿?ŠÃÞúg]ß=•‹ËýZ¦=²j°Â2žµ?ð=²j°Â2žµ?JÏZ ±)ý?H¾5€ü^?ïùL)ÍÙ?H¾5€ü^?ZfÎmò-þ?zrðúé¡?ïò̘ÊfÁ?zrðúé¡?''†—?atɶ+óf?ïµ¹‰½È<?atɶ+óf<f
,U[²<§æuË1s?ð<§ð'û0Œ­PSR4FGL J1810.5+1744?éCr2Í\À@0ÏîÑížÀ8(Àéi¼À;›I²Ñy@fúÅX8@Øu'ST;?§L&Ÿ& {?҆µ¼:…@%p÷…@ÖoºÜµ?ì÷ì5Gài¿Üd…üðJ¿ãÌ©C6Œ¿èä"ŸR¹¿ìô#ˆ›D•¿ïó!3FPSRPSR3FGL J1810.5+1743PSR J1810+1744?‹›ªßü?Œc¥SÓ?W«¸€?Œc¥SÓ?°ˆ"óôWK?²ÉƑ'?íîíaJ{W?²ÉƑ'?Ê[tÎf³q?°e‹3Ë®?éi"ÌfS$?°e‹3Ë®?"ÞpÑ2éà?ƒ–œK¿ö?ïay­bq?ƒ–œK¿ö?'QnŠ?®lLn¦?ﶺH)©6?®lLn¦?ŠÅ_Î¥G«?'Ý@p/(g?ï"ê€Åjá?'Ý@p/(g?§z‡­úGÜ?Ÿt1Ðé"A?îˆW"÷ 2?Ÿt1Ðé"A?/ˆaµÉ?$}oK?ïþ~	×U?$}oKPSR4FGL J1811.3-2403?åÚ¯T}ÀWg?ª9ûÀ8µml%QÀ:'
©§-×@ ?z¿8å@{Ú¡¡¥Ø?Âü$©,µ?DZéDŽc|@±B³÷+?ínÀ	šÞh¿îÌÂn¤ù?êðL-Õü ¿àÞ	|¿æ°¸.°´¿è‹X=®·8¿êGM1:ÇPSRPSRPSR J1811-2405?çËí L?Ч'?3?ÑÉâh%¿h?Ч'?3?ŅÉÝHò?Æp˜·zá?Ɥˆ­ýÃ?Æp˜·zá?â36Ÿï?¶Â(¬Ð
Í?ۙ'Àü#?¶Â(¬Ð
Í?ÄÁ>]L¦?¬2O‹9?êÏ°h¬Ö|?¬2O‹9?Ê:É·eÿ±?ÒhÐãK®?éqM'&€?ÒhÐãK®?'\[ÿî"?¥³Z»S?ïm ˜Œ?¥³Z»S?ÙÚ*»6ï£?¹Y[sÀ­_?ãê¢dˆ/?¹Y[sÀ­_?y'¨Õ¢?m–cÒ¾º?ïÌû𕘝?m–cÒ¾ºMIXED4FGL J1811.5-1925?È$Pj¿×$2#é".À96"4ÕËÀ:z&­é²·@!Ë仯@"Á¨¬\?âA{_ò®ß?áL!¬"2Z@«ã	O4@Aý#,?ç…"~°	¿ïB-¡ú?î•TûÚ×R?ä˜Wz:¿ä…"ÿ‰b•¿êî~F¬ãPSRpsr3FGL J1811.3-1927cPSR J1811-1925?æJ)¹"=?Ò·<?©ì¬?Ók¬Œ÷…ï?Ò·<?©ì¬?ìÍßhÓ ?Ädw:–vF?¿Y'¹g?Ädw:–vF?å˜#ªÕM?³°ÙP.?ÔϸªUÿf?³°ÙP.?ëBIÖZ6¥?­e!î0X?Âöئ—%m?­e!î0X?拍«5?˼Í	wfÙ?ÒèäáÒ©—?˼Í	wfÙ?æ'Ë£›¿Ó?я
—øI?ÒÜh¸È€Y?я
—øI?ç'Úì±TÝ?²½'hNÉ?ÐÚJ&VE?²½'hNÉ?åÙó¸O?ÃLE¦°áè?ÔL÷aÿ?ÃLE¦°áèAGN4FGL J1813.4-1246¿¡Ãã9Îú@Š.ÝcÀ6×1ªœ÷À:O"}Š@öÃì(ˆ@?_[°)ÿ?'D$z¼<d?Ôª±ïÑ´"@<ÜÇÀôQv?úû]ƒé¯?Øhà¿Ô¿Úâ'[â©Ù¿ä²)³W°Á¿èѵ¿¿óö¿î2ò yI¿ïþ Eð¥PSRPSR3FGL J1813.4-1246PSR J1813-1246?woŠJnÖ?‰+÷y?ïÑ!æã,?‰+÷y?‰]æ´Ii?'"F,X?g «º?'"F,X?­áÖË'8?¡›Dğ?î!â"]•\?¡›Dğ>Lòˆ·‡>[¡7úhlV?ïÿÿùK*>[¡7úhlV?\'úè8?q;³Nê?ïñì{‹3?q;³Nê?X\	ۓì‰?nnbC¡?ïóÑûN¯)?nnbC¡?¡à€«-#?›(ʧîÿ?îá÷õM'.?›(ʧîÿ=~/½Íˆ«=¹yñŸ¡Ù}?ð=¹yñŸ¡Ù}PSR4FGL J1814.4+3132¿Ú8œNT̶@5²køvŸÀ:LsGyBÀ<&_ċµ«@iº-ã¾@÷òeÊ?ĬÂkIû?àW.ºþn0@±¬Þü+@†Ð.C¿ìw6b'œO?Ԁ÷Áíö"¿á³p:$¾ü¿ãˆáá¿îÞ>s³¿ïòýƒMýºPSRpsrPSR J1814+31?¨D¥	@?´ÆŒOóÍ?î{¿*2Œ?´ÆŒOóÍ?Îͤ`ûv?Åuç/F?èL–çÁ"}?Åuç/F?Ðyîi»Â?­ˆ9j?çþÃË"?­ˆ9j?˶ÊÏ>?©¿. ô¤$?é=þRML0?©¿. ô¤$?få3eÓ'?gû3±S¼?ïéÌÆ'þ?gû3±S¼?¥xæî!‹_?¦$·…Âì?î¨qæíŠ?¦$·…Âì?ªä ©ØPð?)¼‰U ?îQ½õ™t±?)¼‰U ?{÷+#"ë?iQ86ê+9?ïÈÕєn?iQ86ê+9PSR4FGL J1816.5+4510¿êò©g0Õ@8¼`ˆÖÔÀ9O¢ÓÔþÊÀ<Hm'ÓÒ{@e}x£U?ý¤y&\‹?°!ñâî¢?ØOŽÞ§«@$­1ã§Û?û˜'©í?åÞo÷ß ¿ÑUU|´0Ÿ¿ÖXZ_=¿åW¤A=b¿ëße‹u¨¿éRlžä²PSRPSR3FGL J1816.5+4512PSR J1816+4510?u†P‰«Ë?ƒ©zTàM!?ïÔó^©P?ƒ©zTàM!?Å	?W6{E?Ã}áb*Â?ê½°*2a/?Ã}áb*Â?²eÁB-Œ?¡iÂe‰˜?í¿3G¼=o?¡iÂe‰˜?‡oí£±ö]?xn'Á¨"G?ï¢@Iq8'?xn'Á¨"G?a™´
¢?a®²Šø0D?ïîfï?a®²Šø0D?£0«xÒX?¤XÆ´'–?îÌõHŽ[š?¤XÆ´'–?Þæu'r'?""Ñ{ß$¸?ïyÌF-û?""Ñ{ß$¸?+ó{ˆÙ1ã?'œBŒèq#?ïþ@ÈG,?'œBŒèq#PSR4FGL J1817.1-1742?æòI0ÿ
¿æ¢1ƒ/ÊÉÀ8Xw…À:žé|/üG@侊ê™@^¯ûÛ®?¹¢e^î;Ì?ÚL®ÁI@Åðáy?ùžv*úÕ?ïzÙâ)U¿Þ×q@ŠØ¿ÞƾÀł¿æe}'%¿é™ ºö
´¿ïÿý`éNäPSRPSR3FGL J1817.2-1739PSR J1817-1742?§Ó?Ÿí?±·É£7g?î'Ï?±·É£7g?«  ÍN(·?²¯Ú³I'?îMýóFšT?²¯Ú³I'?ÐK°¨
d?±¦9D8?çÚ'ÿ«úÎ?±¦9D8?¡)
aï?"ç‡*"¢Œ?îï¾Í8`!?"ç‡*"¢Œ?\=ó&ù?Sj/Ï8}?ïñáž2c?Sj/Ï8}?qÛÒ¡gŒ3?{=Õ¿_ßã?ïÜHZ·±ˆ?{=Õ¿_ßã?±œu¹bM?ªþ=÷Ì?íÌqHÓ¿–?ªþ=÷Ì?LUOäŒs?;¢$º'?ïøêœqÄ?;¢$º'PSR4FGL J1823.5-3020¿î43ÝÀŒˆ¤~ÏêÀ8üŽ~³dFÀ;ðåÍNÒÌ@H"Î;G@4²ú"¯u?­‡€sw?ÒãÚzµRÞ@ C­Ò^Ý?îŸ)º_¯?ؽa4"¿ÙØWdÀÉß¿à8lXï¿ßÓ~—µ"Ë¿íÔ§¢òu¿â#ÎÜq…~PSRPSR3FGL J1823.7-3019PSR J1823-3021A?Š0:ù?°PÊ}$4?ï—?Ô?°PÊ}$4?µËW"ZÉù?½I‰'(?íF•=­?½I‰'(?Åa 
^ä?¬q·07?꧷ü¨?¬q·07?}!´N\t—?i yÿi¼æ?ïż—låÿ?i yÿi¼æ?¬Ï¯ÑÐ}í?Çrc6}Œë?î3ž?ò?Çrc6}Œë?'t°H`*³?¤:½øëÛþ?ïlZ}"Ã[?¤:½øëÛþ?¯ò~6aœð?£ &¼Ý_z?îØŒ'Á?£ &¼Ý_z?c°éW»x?)Ô"=çô?ïÿâ}§å?)Ô"=çôPSR4FGL J1824.1+1013?ÊÖ\'k@%NÉ:qÀ9»Œƒ"_À<tЌu@Hkԏ@c—>?½ø^öÛi?Ö"›Á,Î@ýKÁŸr!?úT"úP=°¿äª|`"Õm¿Ú_3Â$RE¿Ü8×¢hË¿áîg`¿î*= ÿ:¿ïþÃNžÊPSRPSR3FGL J1824.0+1017PSR J1824+1014?¶¶?GË?µýBf¾?í)?½ÁRV?µýBf¾?Àžþ{y%¹?½ˆJ^?rÔ?ëØ@a!¶'?½ˆJ^?rÔ?̀¿aíÂ?±"±ôœY?èŸÐ;'"?±"±ôœY?Óâ3%ò-?®7ù'8ã]?ææmé~?®7ù'8ã]?ŒùY§ùõ?±DTGôÄ?D›L?±DTGôÄ?Ìu-x?—ß›ª—£?ïQœÒô?—ß›ª—£?•¨Uìh
?ˆ¼±$9?ïR½Pœ¿X?ˆ¼±$9?—8ÂH¢K¾?"&¾nDJ?ïF9íƒóâ?"&¾nDJPSR4FGL J1824.6-2452?§sÏÙbÀfÕ °åÀ81Må"À;6ÕÓËò@ùmqÈoE@=">5ŵ?¬Í`né?Ößf'¥"@$\_|gZ@Ø¢' *?ìå€UÐÂ?Ëoä¿\̵¿ãN'¯rHó¿å*lO´s:¿î™l¸þæ¿×·b|×ÂPSRPSR3FGL J1824.6-2451PSR J1824-2452A?DØyß(?L´ˆñsP?ïúÉý1?L´ˆñsP?¦ó0ÈK"?­åCbÁ›_?îÌóR?­åCbÁ›_?®ý—¤Y¸™? /|Ø3Vp?î&…È"æ? /|Ø3Vp?‡VF³Ê?xaãúƒ?ï£ö§'©á?xaãúƒ?\dÁ|2ê²?eO)®>`?ïñ͟|ÿÒ?eO)®>`?x—2bÅ?†OrìÍu?ïÏÖÑwEK?†OrìÍu?''=?'°êAr~1?÷ï ›?'°êAr~1?ÚmKzì?í~	6Ÿ?ïÿÙ#ƒy?í~	6ŸPSR4FGL J1826.1-1256?î¢`_'5¿ØžžôÀ5°¦#뗓À9:FÖ~&w@Šp8ø,@Ú j™Ò?•4Ú¼P?ەn¼¡0'@@ÉrGE8ï@ùF'¤?ïþ"ÀC§u¿Êzأŗy¿àüDôü–¿¿æ"x'Èœ¼¿íøMïwÀ¿ïÿÿ&¦³PSRPSR3FGL J1826.1-1256PSR J1826-1256?}'è¾ÝƒN?´ê³1ƒ U?ïÄÚ.N
ê?´ê³1ƒ U?‹'›i"?"Fò,ئ?÷ù:?"Fò,ئ?•z	Þ•'?•H%J̳Ì?ïT/°Øá"?•H%J̳Ì=ýá撼à><-t»á}?ð><-t»á}?¨®ÀUÉ?ËU0Þð?îxm?ËU0Þð?Wµ…Ú?nÐJa¡P_?ïô%9S|?nÐJa¡P_?"ß'¼^Iõ?uŒ"%Í?ffi`ó	ø?uŒ"%Í=ž+w¿=> 8­áoÁ?ð=> 8挋ßPSR4FGL J1827.4-1445¿Ç
óŒîÕ$¿ø<äŒ×êÀ8cã\[J©À;+ÞUõÖ@Y\·Ý@m²¥Ú¼?¿K¸ÿÕ&§?ïÿójÆGx@#ØÛÎÈO@udǪϿâMš¢®R?ï9žÝ%`¿Ê²wa
†í¿ãÝek"£'¿ïùãñ¬€&¿ïþ䬽bÌPSRPSR3FGL J1827.3-1446PSR J1827-1446?È
[™j?1è$ÚÀ?ïÿ¿a™?1è$ÚÀ?ž,gT?£ÀçKµ'm?ï>Ÿ«Š?£ÀçKµ'm? 5X`ñÛ?•NÿK?îüªyÕrÒ?•NÿK?7äÐùXØþ?%Ì%tY	?ïýe²ƒÃ?%Ì%tY	?]I7`"WS?•Ú4:¸?ïñ[d!4%?•Ú4:¸?põ@kxq?'Òì8hü?ïÞC,%?'Òì8hü?šIêT«?–<LU{Ú?ï-°¬›:?–<LU{Ú>ÐÆ:Éb&ä>Èø1 "c?ïÿ÷
 >Èø1 "cPSR4FGL J1827.6-0849¿íÁ©œWJP?ótx]ï"À8E`؇ëòÀ:¶6eÃ@s¶0(@¼>	P?´A? ¸m€?ǸTÝ¡±@ÿ¿ž ß?óôÃ¿ÒçƒÝD¿?ïðÏ@D"®¿ä¶ÉöX·Q¿ä±F^‰"¿ë:¢hJA¿æ"ÌàîÂÁPSRPSR3FGL J1827.6-0846PSR J1827-0849?Ûr(ë fV?Ϩ>ãjž?âFëŠ/ÌÕ?Ϩ>ãjž?®hwHòô:?²/ÈXi¢?îx‹pм?²/ÈXi¢?âžoɳà?´ònÊ'Ù?Úà l˜?ä?´ònÊ'Ù?²ó+-Æ°Ö?—ë~Õo´?í¡šš~#¥?—ë~Õo´?—úáRØÏk?žÞçÓú™?ï@(õ 3D?žÞçÓú™?yZ!{Ô y?ˆ]$¸
á?ïÍK½6÷?ˆ]$¸
á?Éߪí ?²"S¤Xi?éˆ;ÕD¸?²"S¤Xi?g çý ?[g(-E³h?ïè_ä°Ýó?[g(-E³hMIXED4FGL J1828.4-1059¿½œ¡izJ§?£1]<F,À7¯<Kà©#À9½Ñˆô/è@^Ä[@¸•";"+?½¡§Z!‰"?Å¡… eÑ@
2†!î?û§)Æwô¿ÜW'còà¿ÍÇNފd¿è.®è¿è‡B_ ¿ìŠ)º
­h¿â–¹‰$PSRPSRPSR J1828-1101?Õ.&³6èc?Ó$UXæºÎ?åhì¦d‹Î?Ó$UXæºÎ?¾æ^nJ`?Àujêsj ?ì?C426´?Àujêsj ?ÜÛñ´I?¶ÌÆ,·¨?á'%Û~8?¶ÌÆ,·¨?ÊþƒFN¡?°A6n£?é@_.lW ?°A6n£?ÀÄòiz~?Íçš@ç?ëÎÃ{%¡`?Íçš@ç?~Q=?ˆ7qþ—l?ïÃ]Ä£}?ˆ7qþ—l?ÑMìX??¶ÙmÆISp?ç~÷Y	Óá?¶ÙmÆISp?uaŜF½?iå¥ÊI Æ?ïÕ<tœ×^?iå¥ÊI ÆPSR4FGL J1831.5-0935¿ï¡ü"¿Œa?‰"ÏväýŠÀ7íèPïÝÀ9אíùm@Œú#G,å@@E]b×?ïd²Â4˜c?ÔEµV¬µ?ñÕ9eQh}?î%eJ´O¿Ëç‡Ù¿å4µê28¿îx8@8TZ¿ï|ŸB¥ìä¿ï÷8EÁ«1PSRPSRPSR J1831-0952?æAʈqK?֑ýÅY?Ó}Æjïk?֑ýÅY?ÓhLp­"t?ÓTŽL´cŸ?æKÙÇ©nÆ?ÓTŽL´cŸ?Þº1©	=?²#Y@KA?à¢ç+{a~?²#Y@KA?‡¶äö<ÇV?‡ù	öáº?ï¡$l4ËS?‡ù	öáº?é¹Ðàq‰?ÒÝ¡‡_ì`?ɼ~9ۈ?ÒÝ¡‡_ì`?´,?öéj?Æ¿¹úô9?ízxL
þ?Æ¿¹úô9?ÞM	óô®é?²ŒÚȧ½ã?àÙ{¨‹?²ŒÚȧ½ã?€j
ü'C?ÕÁ¥þÁ?ïÿþic,?ÕÁ¥þÁMIXED4FGL J1832.4-0847¿âˆqýã	?ÇÔeG'u'À8¡å$w¯À:áî¶+ ˜@ºÑ!Vî@U™Yعj?ÁѨi@5z?å×p>×V>@áµâ¥|&?ÿž5e§?ßî*Àr÷C?ãµ¾=gêu¿Þ5B,Oê¿á¾QtfÚ*¿íáv<?A¿ïÿè«î0PSRPSRPSR J1832-0836?|P(?‰?ƒ7*‰wÂ?ïÇÝ_þ(¡?ƒ7*‰wÂ?¦[Ç]ïkÖ?§o	#~?îšC‰ÜQ?§o	#~?¼±B¥
?£IvqšxÇ?ì|	׫^N?£IvqšxÇ?•M
Rbž<?|ŽH¯ˆ¥?ïU—•C¯¾?|ŽH¯ˆ¥?P8Gyæ?RׇŽÐ?ï÷ã¸þ2?RׇŽÐ?wg)wá¤?†c³!®?ïÑ1ϗ½?†c³!®?'oQ¶DäÐ?…;*¦ÜH!?ïl…rMØÙ?…;*¦ÜH!?NN
`Ëi0?@~ÜìöŽ¨?ïøl|™ÈW?@~ÜìöŽ¨PSR4FGL J1833.0-3840¿àÕÞ"#…/À*€d©ÍÄÀ:¬îÐ,ӞÀ<£éå‡ó@Z­KR8Ý@5Êd{?ȽÊ{cÏ?à%ô»ÿ/@î­ÕÀ­@{!]æ–?ïã.qÊH?åòØ?ɵ¿Ýè{Vb¿ä Ï§Æ¿î‰›ár¿ïÿԖũÃPSRpsrPSR J1833-3840?ìQTf½+ù?¹»˜X74Ü?½u\Ê <?¹»˜X74Ü?éß,5hÀ?Âø=ؗu?ȃO*_¥?Âø=ؗu?æê	<?³'©"àf?Óü+ûí‡é?³'©"àf?ê՟»‹u®?¡´'vóAû?Ä©Ò)G?¡´'vóAû?á›	Ý4µ%?ËtAŸ¡_P?ÜÉìE–•·?ËtAŸ¡_P?Ô1OT(C?Î:«¢…¦s?åçXxUëß?Î:«¢…¦s?È£†""¬V?±@&<¨ól?é×[ë?±@&<¨ól?Õ£ÈuéÕá?³CìÄ»?å.Å?³CìÄ»MIXED4FGL J1833.5-1033¿ìW'F¿ëù
ãˆÐôÀ79€C‡>MÀ:+-û»Í¡@—Э'Ñ@v¦ã.8"?§IÜÂ?˒Où<—`@ H,nóÓ¢?ñ¹Z¢
¢?ïúGߒ¢/¿ËYý¢W®=¿ä>ÚÑrMû¿ç
U=Ÿæ¿ë
+ãðU¿ç_QŸ/ÐPSRPSR3FGL J1833.5-1033PSR J1833-1034?…¤mµ¢Y?X0. BÎ?ï©nKÀ¦V?X0. BÎ?™ÙœŸû‹ç?žÌ㇟'??ï13ÖèQ?žÌ㇟'??Ì'¡—óYÝ?²ÌÇá
!?èöš)‰?²ÌÇá
!?VE[9Æ¥?CÈ¢…\ü?ïôÝR‰˜M?CÈ¢…\ü?t4ŸÜŒ-?­¿R†Ö6?ïÖ喌Ø?­¿R†Ö6?lÏÀ^â³ô?~¶ð'>?ïã0?җ¬?~¶ð'>?¢|cË"õñ?šÉ€añ(û?îØ9ÃMС?šÉ€añ(û>çN0ùµ>áJng
ÿ?ïÿè±Àèú>áJng
ÿPSR4FGL J1836.2+5925?ãŒÛ@­ð@9(€QÉ÷À53¡Qô¿ZÀ:}àÖo
@ºMϖ«©?þ$Ã9¦?X±ÊåWb[?Ù=¤¦=@_jcÇOµ@)."?½ÒfÛ)1¿ÀËFý¿Ûοì¹ñ¿åùèÄzô¿î¯Úê¿ïÿülòPSRPSR3FGL J1836.2+5925PSR J1836+5925?f¢y,aÜ?g¾âSÌ?ïé]†eV¾?g¾âSÌ?‰Fqҟ,?"³•)ƒ˜7?ïšåÂo¯C?"³•)ƒ˜7? Ĕ²
¶?˜!²)êQ?îÿ3¶Þt?˜!²)êQ?ð?^fÁý|GB?P­{Ìô?ïð̟!?P­{Ìô?_ðë£ô.Å?už2‡ö?ïðŠ
	©?už2‡ö?gÕï)Q?‰zņ÷?ï|Ç15	Ö?‰zņ÷?ðPSR4FGL J1837.8-0604?åBQœ/î?Í2¦ÆRàÀ7èȼœÓáÀ9¬DmŒË@ W\ÆT¡@öÙæÃ1?Áþ‡ÚÕN?Á8SX—›¾@t#¾K)Ê?ÿý`Îvðø¿åÒJO¯j¼¿Ö™5{aö¿à×:yx'â¿èRœðf/	¿è»°DÖɦ¿ë"^~»qÜPSRPSR3FGL J1837.9-0607PSR J1837-0604?áS*Òf"µ?Ô\#»à°?ÝYª[2֗?Ô\#»à°?Ý´>T¾7"?Ðî`營W?á%àÕ äo?Ðî`營W?ÛPqG¶?º_GŸb?âWÇpÜ$ó?º_GŸb?ãÓZç"?¹ÍzzM+µ?ØY×J1Ú÷?¹ÍzzM+µ?ǵêùï«Û?ÒV»iô?ê…A"	?ÒV»iô?»a~hChé?Ď`&A™d?ì"Ð2÷'ã?Ď`&A™d?Ӎu—dh¾?Đb¹2¼?æ9E4MË¡?Đb¹2¼?±4µ£TGD?¨òÀÛµšm?íÙiKÚ/G?¨òÀÛµšmMIXED4FGL J1838.9-0537?Èï7t¥2?ÉzH†µˆÀ6é]…UÀ9¤ßI® @ lëT¢C·@÷é¾u5?­%Åask?Õæ͓œ*@'ڎO¹{·?î}Ððóȏ?ïh—c^t*¿Ý¤¯!k4¬¿árÞyzпãORúȉ¿ëÖWûi˜J¿íCèWlÎ_PSRPSR3FGL J1838.9-0537PSR J1838-0537?Œ·võ
ö­?·ëÖaÒ×?ï"$9'•?·ëÖaÒ×?"#~ÜÀ:?—«É›4¼Z?ïfä	C9?—«É›4¼Z?±Y³Áâ-Ê?¥¤¼.Y?íÔɇŒÀ‡?¥¤¼.Y?v°s(|
>ý<š©¾e?ïÿ²%4J">ý<š©¾e?¸h'UHJ¶?Òa¿nüs?ìòû>z?Òa¿nüs?f»ùTçü:?s-àäC€?ïéD•"?s-àäC€?'û%…[Û?	ù¨øÝ!?ïh'îÓÕ!?	ù¨øÝ!>q5^,òö>qyi›|?ïÿÿÝ£è0>qyi›|PSR4FGL J1843.7-1114¿ïót6¼2SÀW=
§ˆÀ8Œ»*ƒÀ:ꨆœfÓ@³¸ʏ@FKùӖ?²Àßٙå?Ô]+ß×Ár@¼ó…@=rŸ.ÙÝ?ïÿºà¼ô¿ÛUçÞK$l¿ç™aOü¿è®¯?ôÖ¿ïÿûÎBÓ?ïü>>ÿðPSRPSR3FGL J1843.6-1114PSR J1843-1113?²Fœx:1?»Ø°Ûª‹.?í·<LŒuš?»Ø°Ûª‹.?¼ƒž|úžä?ºTvÂݓL?ìoŒ0`¬#?ºTvÂݓL?ÛÜÝ©ÇlÄ?¶ä~'¢Ì–?â'+Iž?¶ä~'¢Ì–?Øwô~þžè?³tO£¥bÛ?ãÄÀ€°Œ?³tO£¥bÛ?ª€M+uÝ?°Ë*uXù?îWÿ‹;?°Ë*uXù?€‰õ¢¸?‹–ÜŠ`êÇ?ï½Ø)f©?‹–ÜŠ`êÇ?ÆL Ä¨ˆl?²K ¤j'?êl×ÎÕÝå?²K ¤j'?‹Ñ<edrk?~ȋyº8ó?3tw?~ȋyº8óPSR4FGL J1844.4-0345¿ëÆTx'Y
¿ÅDÜþÉBÀ7ˍ¶6ˆRÀ:|TŠ›ÏÕ@ùà×Ù@ÌÕeø']?µ¬]–‰î?äï »ç¢@&W?·¥ô@8g'›%¿ïîB_Ëí?ï[Á&¦\ö¿ØÝ>|¿æàzÉʹͿî»ûXÑRn¿ïÿl\I¬òPSRPSR3FGL J1844.3-0344PSR J1844-0346?f›@ÊjÞ?wF÷Ó\?ïédãâñ…?wF÷Ó\?—‰"HÂK?šÆO'Cž?ïG[¶ßû~?šÆO'Cž?¬ýÛ{zðm?žèF㯶h?î0"H:'‰?žèF㯶h?aôKç>#
?R§\ wz?ïî´B}?R§\ wz?`/ÿqÂ?'/´Œò?ïïÐíî°w?'/´Œò?k.ÐÆT)L?EsgV×w?ïäÑ/ î§?EsgV×w?IhˆÏº?"י߃–u?ï´¿‡6b?"י߃–u>îš.c­Ä>åЁ0×sã?ïÿáeúÊ{>åЁ0×sãPSR4FGL J1846.3+0919¿ï¢¯º9Ĕ@jš^»w:À8‹ÛYÀ;¦1Wà@˜–t¸@xs€?£×r࣢?à¸põ5¢@2Ôm?ž{@¤ŠM÷.Ë?Ëìւƒ(¿ÉîNý"õ¿Õà3œd¥¿â¹q:Õ¾ä¿îD žq¿ïÿlÞfþPSRPSR3FGL J1846.3+0919PSR J1846+0919?o}m+æŽ?t¿÷í°ô´?ïà''¨ÿ?t¿÷í°ô´?"
BÈLk†?še];•8~?ïg•é"aT?še];•8~?¤$üteV?™Qn'ëì?î½°8±;;?™Qn'ëì?Ñ*À]mß?r4Ðm³Œ?ïÿyv¨AÂ?r4Ðm³Œ?n'.½kÿ'?}çPeVô"?ïámÑÙQ?}çPeVô"?hõ%†wRó?te´l³!u?ïç
Ú4Ð}?te´l³!u?œßÃç¤S,?–r؃œÿ–?ïà™¢?–r؃œÿ–>usb&eËÞ>€½Fúáò?ïÿÿÕâ<>€½FúáòPSR4FGL J1852.2-1309¿èÀi´qÀ"ý>" 
À:#º
RiYÀ<'@ÿ¥@žD 
é?ÿb‰,d?Æõì€Ç:½?à=òÿf}@{ùiãÉ@\u'ŸVG?ïö.Åæ(¾¿»òªÝ¿ÔH$ÜÙ4¿âg$ÒG`¿ïw^3'þ¿ïþº…¢kÐPSRpsrPSR J1852-13?ݧëÙyÐÉ?Îý"BÍã?á,
Cœ?Îý"BÍã?օeHóӑ?ÈNµ¶–æ?ä½M[†8?ÈNµ¶–æ?ÝtÙÞO£y?µ:*™í¸'?áE"Ø.D?µ:*™í¸'?ᦒýYmÁ?®úq‹›p?ܲÚM$?®úq‹›p?²!MZ¼\?²k¢}l§?í»Ö]`¤?²k¢}l§?¨Á¹>Âý?´Ä
m5?îsälfð?´Ä
m5?­KNô4?œfß&#|È?î/;K{/?œfß&#|È?ÀyASÓ?¨Ùø3¡ÐÇ?ë᯿9«?¨Ùø3¡ÐÇMIXED4FGL J1853.3-0005¿¶¨FŽ¥aÞ¿Þz5›mYJÀ9 òxXrÀ;"!\q@ "Dû݆ƒ@–ÖZ²Ô?ÐoÜ†©'?çFz7Ԃ¤@Íÿàè@g ÎN¿ïÿõEq#?ïÿÙÔóü¿¼¸j•6|¿ÚÌaÿÏ¿ë3g5™?¿ïûÓ {‹PSRPSR3FGL J1853.2+0006PSR J1853-0004?Ý~=¥Õ½?ÑP'ÝH"·?á@áy­!?ÑP'ÝH"·?ÖGÁ¸ÐD?ÐtTkEù?äÜ#—ðÞ?ÐtTkEù?æIě¿¨f?²"zÐõ‰+?ÓlvȀ¯4?²"zÐõ‰+?ÖÍã "ö?¶zg¦t¡Ò?ä™p/î…?¶zg¦t¡Ò?²,nÝ~+ò?¹+˜›S?íºr$4½¢?¹+˜›S?¶{®ë"V?ÂLfHfÿœ?í0Ÿj>U?ÂLfHfÿœ?Íkný¨{£?¶p–—MèU?è¥$@•á?¶p–—MèU?¨¾æŒâ3?âÇôd®?ît—#"ý?âÇôd®MIXED4FGL J1855.9-1435?¥¯Â¾À•hÀS# îøqÀ9ò".E©À;Ѿâ(~¤@€ô2}@3•#SÀ?¿.æâšœ?ÆӘ•±ƒ@®p:û~'?ýQ§Ù"q?ïöÅúJ´Y?薘ȹAÖ¿âê¹çíºƒ¿ÕÜH)¿ìD~‡Å\¿ïÿ*¸:n'PSRPSRPSR J1855-1436?îÄ>eìC
?©5!}†Ç
?£¼ _èe?©5!}†Ç
?ã¯H\\™«?Ì?Eßº?Ø¡oGFÌ©?Ì?Eßº?ímtfü…Ä?¡1}͍`?´"\ÈÑÜ?¡1}͍`?ç&ã´ùO?­$ÜS3¡?Ѳ8–
a×?­$ÜS3¡?ærŠp¼x?ÆÔ¾!¨
?ÓëÀ‡?ÆÔ¾!¨
?ÇÚϾ]?ÈdaMö?ê	Lhœ»?ÈdaMö?ç;i|_:è?µÆÆ'H»?щ-AŠ0?µÆÆ'H»?ÐCL=ù¾P?½'j
µ»Ž?çÞYá Ø?½'j
µ»ŽMIXED4FGL J1857.2+0941¿ÆðE=ÝíB@ñ|ƒ^À9B%ÁZ¨ÃÀ:àãܳʝ@=ø9âû@þ¥2?Ë°›=އà?Òõv¤¢X@÷Eî Ú@½"ñÙÍ?￶Ï4†¿ÜœiÌ2ô¿é3Î~}´a¿êæÿQ"W¿ì4q ԋ޿ïúFsBîPSRpsrPSR J1857+0943?íHy#µð?¾-ñªÒ§?µ¿Ä8,*ü?¾-ñªÒ§?ØýÁ)‰ö?ÌMęwŠÑ?ãk;s…?ÌMęwŠÑ?éˆn<YÞª?°D,󱛢?ÉÞG˜…Y?°D,󱛢?ãXqü?±ÞymÎ;l?ÙÑñOõ?±ÞymÎ;l?Ý1¿¸	?ÐVÌH 3?á|ç #ü?ÐVÌH 3?¢–?-M§9?¬æy`û)?î֜
+%Œ?¬æy`û)?ÚÃ^t)ˆ?¹;]gþÛ¬?âžPÅë1<?¹;]gþÛ¬?ªÖl7$ž4?–4kNæ_?îR™<Hýí?–4kNæ_MIXED4FGL J1857.6+0143¿éü%kc?¿âÓ_XU+«À9ÐQ¼‹6À; B\›âI@ ìÓRwò@'ß­*p?Í@zï_t?ïÿ¤€RuÄ@r²žM]?ÿäP\8åû¿ãú=‰Mq?ë÷u¢™r'¿ÙÓ7º¿åq"ý€Hæ¿ð?ïÌ+òÍ–PSRPSRPSR J1857+0143?qwoj†¥?8æ=b?ïÝ! È3?8æ=b?¨8Ne"­œ?­¥0vvq$?î|{ë}V?­¥0vvq$?Îäí?‰ò?¯Žô¯QØ?èFÄ°¿"?¯Žô¯QØ?'æûÒ½?|…Íäîº?ïhÈ':pX?|…Íäîº?‡5ìÖ?'Æ?²ÛÝmÑ65?ï£(L‹…?²ÛÝmÑ65?wðxöNaö?‰QØÑ(H?ïÐ
üä?‰QØÑ(H?°‡Ãã? õÍ#Ä1F?íïƒÆ¸P? õÍ#Ä1F?4¶'ð¿/?)[$Np?ïýi-§>Y?)[$Np	PSR4FGL J1858.3-2216?àÙ҇nSÀ&ÉE•5†ËÀ96$)ªô5À<.wîN&Õ@÷ýÙµœ@ɪ`':P?²»dš‰X¯?ä:¾ÖêÞ@)¦XĽ4?ú¶ÛʚC?ïî"ã)/¤?Åvpõ‹‡Þ¿ÐYÏêŽ~³¿æØßT¹Á¿î @gNC¿ïþY¢2ÅOPSRPSR3FGL J1858.2-2215PSR J1858-2216?1šó.?4.(Tƒu ?ïýÍìe! ?4.(Tƒu ?¨¢q3±§?®ª·7??îuØïÅË&?®ª·7??™µ8›8;?`®ã8'?ï2Wþ;&>?`®ã8'?6Ó N΍d?.Êk²½?ïý%ŒnÛ?.Êk²½?I°:Ä?PGøôœ$?ïù"üe……?PGøôœ$?Šßö›vÊ?˜PxGÍ9¨?%\äe?˜PxGÍ9¨?ˆÝ´M:u'?pŸÊÄ2—%?/é?pŸÊÄ2—%>ÃCuÐeï>Ãf?ÚD÷1?ïÿû/X)¯>Ãf?ÚD÷1PSR4FGL J1901.4-0126?È]qkÊvÀ¥úÐìÀ8©@GDbÀ;Ðzw@ c°(§>@™,d?°6{<6g?Ôz …2`@µGZ1¤¾@ƒG#€Ö?ìÀÂ}h‹…¿Ìo`¥aÏ¿àÛ¸•Ò¿å#'†Wv¿ëò"a¤	à¿ïÿÿ&¦³PSRPSR3FGL J1901.5-0126PSR J1901-0125?†3mj¼Œc?–Q€ÖÎ?ï§2JUŸ?–Q€ÖÎ?«Œ‡,A—ô?¯qê¦m
Ç?îG7«1?¯qê¦m
Ç?Á¨-ÊØD¿?­L›·q"ï?ë•ôIîÐ?­L›·q"ï?Ã*5Ú=´Ó?£(©Pø"G?ë5r‰p'Ë?£(©Pø"G?YÅ£ºd'b?S)@ Ä;?ïó.0D?S)@ Ä;?|Rg'lÒ?‹ú§Tí?ïÇ[1»7?‹ú§Tí?…¦Á&N¾í?vuhrgI
?ï©dû'Aä?vuhrgI
?{­þ{Q¢8?g‰ðDNK+?ïȤ˃Ä?g‰ðDNK+PSR4FGL J1902.0-5105?ïâÿýYe*À6`Yž×ÇÀ8'hŒ±SËÀ;¯ð†nD@óœR†Šž@1¸YxAZ?¤—XP µ?ÑòñCú€º@(·×<'W†?ÿQK¯€á'?ìô'ßíæοÔíï\C͵¿ãÕ¥ÿ-¿æÌ£FÁ…q¿îß5/7¿ïýG¾Ûr'PSRPSR3FGL J1902.0-5107PSR J1902-5105?zª7¡ÙæZ?x:uã')?ïÊ«Î*+?x:uã')?ÅW(ÛÁ?Á«Œ1@?ê¸xª5É?Á«Œ1@?¸$aÐëÅ?¨%Ñê:h?ìûsŹL?¨%Ñê:h?x¦ÛÔXó?nºûÅÜä4?ïβIáþ?nºûÅÜä4?nV67o?fÞs3'?ïá©Éù™ñ?fÞs3'?¨c¹m1?©k›Ò«th?îÏÉßæ
?©k›Ò«th?'"÷05˜a?ˆõÓ]3¢?ïvèFGY}?ˆõÓ]3¢>ÿƒ#™Ù7R>üW+8œD?ïÿÀùô'ý>üW+8œDPSR4FGL J1903.4-7053¿æÚ?¯îÀ:~¦Á HàÀ9øy5v'À<ºø6#@ŠøEÌgø?þ{9wÑ?·>,á_€ï?ã'Èâ\@!$¢v·í?ÿnãMß¿ëj2±‹(¿Å¸À¦MÝ¿ÁîŒe(£¸¿àfN²Š¿í™ÀÀú܀¿ïøÆ+$qPSRPSR3FGL J1903.6-7052PSR J1903-7051?ƒáç09Ou?'¢Ø·°"?ï°xcÂ?'¢Ø·°"?ÌcŸ¬Ù?Âßہý?èçÉ» ?Âßہý?¾³p9ë£?¨¡KŠZ?ì)'ü8Œ?¨¡KŠZ?ÀùöÀU?¤à뀫±Ö?ëýû'Oë?¤à뀫±Ö?ÃîL%"Üh?ÖvÂAâC?ëlöšÈæ?ÖvÂAâC?¯èïœtY2?®d"–YE?îqô=?®d"–YE?¡‹u½¼ü…?"}6'T?îçH¤³X?"}6'T?rLgS¢œ©?dZ!ó'Ó?ïÛg1't6?dZ!ó'ÓPSR4FGL J1904.4-1129?à]´‡l׀À $Ï®ÿ\lÀ:ÇnìFå˜À<dÍßòC@}ÂuÛÏI@£°#HÚd?֋Óyq?ãRE|áÒî@~zÄÂ<P@¾ÒEå?åŠ)ýýÇ¿ì&á`'¡°¿Ôöǝ
"¿è€ôËۿïÿþó…õ?ïöÔþIœPSRpsrPSR J1904-11?ï%,|à¦H?›ñƒ
Ü¥?›Zpcë6ð?›ñƒ
Ü¥?í˜ÀC…Œ?·v?
º•©?³9ýã×;¢?·v?
º•©?ìâZIìð?¡¼i-d=÷?¸í-¸œ'?¡¼i-d=÷?íäî\®F?•O]í8Uœ?°ß(‹Ð³U?•O]í8Uœ?í÷ûo€&?²Zo°Ñ"i?°@$'µ4Q?²Zo°Ñ"i?Ó/úú1´Ù?Ðñ˜IɈÜ?æh'ç%"?Ðñ˜IɈÜ?é§@n/2ž?°¿z8Ê.´?ÉbþGC5Š?°¿z8Ê.´?â_ë'Í·?¿ÌW1J?Û@(Üd'Ç?¿ÌW1JMIXED4FGL J1906.4+0723¿í²ê\™wÐ?¬)¹úµÀ7Gg"s—§À9ÝZ±&~@ÔŽþ
2@%¸ m]Ñ?°Â÷Æ´?ҘnáµD@%Ԗ$š@°6ú*O¿ïcÔ?ïø{§@KJ¿å4>vn¿æº¯ßV¿ì£¶ôs®¿ïÿ#+~3PSRPSRPSR J1906+0722?ŒÊÞZõ·*?´F°7.¯/?ïŒÔ†¡ç"?´F°7.¯/?›D¨Ÿžõ?¡YÛ¢)jo?ï%ÚºÌI?¡YÛ¢)jo?º˜äŠP?¦ša?µøu?ì¬Lãnµü?¦ša?µøu?To
9•Ô?J.c8?ïõÈzòS^?J.c8?¦+èßNšó?Å
蜝@S?îArÔÁ?Å
蜝@S?jõ¾ ''?vYåÙYì?ïå
Aˆœ­?vYåÙYì?¦©.—U?›ÆÏůà?îŸÅm2?›ÆÏůà>ωïN¯™<>Эˆè|Ù ?ïÿø]ˆò>Эˆè|Ù PSR4FGL J1907.9+0602¿éO'X8¿ìÔpÄÜ>À5äÜÊpÑúÀ9¾ÕöA:]@€Î(™Ò@Y9W9£?€×@ÕCz?Ó
Žÿä:@?Ÿ‡ð#ê@A‰Km¼œ?ïìu¿I×e¿Ô€ä+Ž#D¿áú@m®YD¿åÒdáÖõ¿ìøb²|¿n¿íãP!U*PSRPSR3FGL J1907.9+0602PSR J1907+0602?IhÞ7€Hñ?Võ'4˜Õ?ïù¥ÈH{?Võ'4˜Õ?ŽÉîn?˜ägW®æÓ?ï"Ù¼|ü?˜ägW®æÓ?PŽÞ‹®M?}=ðó?ï}{ˆâg>?}=ðó>A"Vhтâ>S5IŽŒåÝ?ïÿÿû´}>S5IŽŒåÝ?Dè¦z»?J¦›Y¶@™?ïúÅú(XA?J¦›Y¶@™?_Ž,#¯'–?j¾Š*˜p?ïð8ê#Â?j¾Š*˜p?'\R¢Íg'?]Îp_–?ﶎµ˜†R?]Îp_–=AIÃz®ù!=pu"˜—†?ð=pu"ä&WPSR4FGL J1908.9+2103¿îåЛ®$@è^ùŠ›À:7ÉÞÛÃÀ<Ó;{×@ÓÇ­©@±¢|—*T?ÄïL>h?Ü¢)` §@ö=Ÿ@Afl›‰´¿Àôš	¿çù5
¤¿«lи¿¤›¿åLx~–ÞÔ¿êáfµN+¿ïÓ	'Où=PSRPSRPSR J1908+2105?äH—&*j?Êeq[…?×Ñnѳ«-?Êeq[…?æz%#ê°?Éöþ¾PL?Óµ¸*¡?Éöþ¾PL?ç†Ë›ÊKh?³úr>§?ÐòhÈki0?³úr>§?êR:Ë`™¦?žOcÕm?Æ·Ò}™f?žOcÕm?Å0ð½É1?Àâ$yÿAá?ê³Ãо´?Àâ$yÿAá?ÈWéx šw?ÈïTK±¯:?éê¡÷Ùb?ÈïTK±¯:?˃ÌØû?´±'Aˆ û?éùÉÁ;?´±'Aˆ û?Ôµ@dÛ2&?²)ÝL'N?å¥_͒fí?²)ÝL'NMIXED4FGL J1913.3+0905?ì˜ÖI3‹Ú¿åñ|‰'öÀ8¯YAºµÀ;0Ž=E@d"iS֗@ñÓíR~?À÷ß`"U?á
&"¿?F@¿b€þ˜@³8•¶Š?îœ"_ü?¿çædžJ ¿Ý %ú»r‡¿äÑiêe¿ïÿôÂ_5›?ï÷ŞÛ!úPSRPSR3FGL J1913.0+0910PSR J1913+0904?bTï	ÔeV?r…Éþ?ïí«H£?r…Éþ?§oÈ]"œ?¨Ã‹–²Å¡?#b?¨Ã‹–²Å¡?ÀÓ®þ°Ÿ›?§Ì¾	:'K?ëË@SØ?§Ì¾	:'K?¦JÕEª?'N{ û±¾?îŸûRÇ">?'N{ û±¾?«93ÓÀ4?Ë'Î'b<?îLlÏ%?Ë'Î'b<?tœ:—+Yc?¥æj=ò?ïÖNJÌ)í?¥æj=ò?«Ô‰š"%?¥6Ö-ƒ!Ü?îB·f¢æ
?¥6Ö-ƒ!Ü?Bq5þ†ÿÁ?:Y|Š‡
?ïûc²›·ñ?:Y|Š‡
PSR4FGL J1913.3+1019?éÏÑm+¸§¿½÷'qøÀ8º(8-m÷À:gþ¬Bê@!¡žJÙB@& }¹i?Â6F¸÷?²n·Ù»s?ù…õB6Ü5@*ívæfQ¿ß`nŸðË°?ïò´BgXª¿×
¼;Ú÷ˆ¿å ø0'æ¿à®2ã'ø¿ç.uÉ°¸šPSRPSR1FGL J1913.7+1007cPSR J1913+1011?ìPI³?ÄMHþKŸç?¿å}·¢f?ÄMHþKŸç?îÕy}´$¤?©#Ö6Ê?¢¨h(-Qº?©#Ö6Ê?èÑRz÷#?²g	»1ó,?̺¶#£s?²g	»1ó,?îi67I˜O?'@"Õ*?©lœ‰®­?'@"Õ*?ë¥Í)>Þ?¹Ñ忦¸U?ÁhË[¸†?¹Ñ忦¸U?ëJ}5F%?Ɲje	Ö)?ÂÖ*ç›k?Ɲje	Ö)?ìjèÔóÀ_?«ÙѲ®¡:?¼¨¹Xaý?«ÙѲ®¡:?ètåͤ¹?µžAQI—Ð?Î,hÉmâ?µžAQI—ÐAGN4FGL J1919.1+2354?ç¦ÚðQ`@å9û¤P­À:µflE£xÀ<Š˜¨ØѾ@ÏÓ)`G@ãŸý`éO?ҀóûØÑ?ïü³åu:?@_–ž<–‰@£º	P¶§¿î«rßñm¿ÝiÚ¤¦½ï?ÞUIž¶™¿ì²ZÆ3¢¿æ¶õ׈¿ïÿѧ' ÖPSRpsrPSR J1919+23?åwüò*
?Ð=-¨.ݹ?Õç«å?Ð=-¨.ݹ?ÓOÔ»H?̄ '§?æXz@¢\?̄ '§?æä´Îí8?³I€ Jë?Ò6—b%?³I€ Jë?ךT¥Ü4?·qäÏYb?ä2Õ­qæ?·qäÏYb?Êׯã̲e?ÈãU'ñêò?éJÓg?ÈãU'ñêò?›ìBîCo?¥fÌ):$?ï èÄá,?¥fÌ):$?ÙXKǏÝ>?¿áºsó†?ãSÚ8a?¿áºsó†?§@øàÕW?š¿ãÞ Û?ðd4;?š¿ãÞ ÛMIXED4FGL J1921.1+1930¿ïO¡L…-–@ÃA2Ð7À:YP¦á€¹À;Ù'æ÷ñ@ 
Ž?w4@Ã/M= ?ÑcꠝCó?â©þk«@~Ó½Ö.@̸
Íóé¿à™æõlÿ¿èž÷ýR%½¿ÛõÀ¥Í¿ÞVe9q'¿íM,Ù|Þ¿êÔÁÔiPSRPSR3FGL J1921.6+1934PSR J1921+1929?á2',˜»?ό\Ø{µ6?ݚۧÊΊ?ό\Ø{µ6?ݶúWõ_h?Ϋ¢ìºº?á$'ÔPL?Ϋ¢ìºº?éõêäv?¯­ÙÐ=?ËÄ(Tn'Œ?¯­ÙÐ=?æê´ã2P?®iëA‡(?Ò*–9›_Ë?®iëA‡(?Ãfû»çf?ÀŽ·8+?ë&A&z?ÀŽ·8+?¤›'nX?«XüĬÚÎ?î¶GÙC¹Ï?«XüĬÚÎ?Ô0ºË¡S?¹¼êä\Wç?å碚/|Ö?¹¼êä\Wç?½F8 '×?©ÏZÁx£?ìW=Xûï¥?©ÏZÁx£MIXED4FGL J1921.4+0136?ïÕjT 'pÀ·rÁ¾{ÑÀ98èÑQ­À;Ù¥J_ @"ãð)ô@÷¨»uŒt?µ™ËÍ]÷?Òù,Ü×ÜË@M;ÞÓ_Ž@×£—'?堟²¸N'¿Þµý½ÛmO¿ßîÝBæ¯w¿ã¡¸LH
¿ë`0âvd¿ïï\ÏõPSRPSR3FGL J1921.2+0136PSR J1921+0137?¤Ð–vr¤Â?·'A™£I?î²ö˜´R"?·'A™£I?ÀbKÙÐÊ?½_ .^7?ëçyí	‹Î?½_ .^7?×t¬܍=?µPATrÄ?äE©ñ'¹b?µPATrÄ?͐·×¶úl?¦²¸UòP?è›Ò
Ae?¦²¸UòP?gŽ<m•kú?\ÌÕf"?ïèqÃ^0"?\ÌÕf"?'Ê ILT?š)šbA£?ïiªýÞ×U?š)šbA£?›cÐH¨…?'—©?ï$á}Ö<?'—©?Œ~
òÍ<‰?uVêökB?ïŽÔyƒ=?uVêökBPSR4FGL J1925.2+1729¿Ûâðåk?æ'ÛçlÀ9ah¼O§À;:²<þŽ@(QغÂ@Ût´?Ê]?5Êè?ä"ûmI@9!ßyx@ÕäÎvE¿ÛxH[c}ÿ¿âÄôÉ_¿á5^Pp¿èõPPx¿í‰"Ô7û¿ïÿþó…õPSRPSR3FGL J1925.4+1727PSR J1925+1720?Ç-z?>âÇ?Å1ÚUÿïm?ê4¡p0GN?Å1ÚUÿïm?´Ñ4ˆWXÖ?·6ʟÿm?íeÙoÓU?·6ʟÿm?×ъûàÐT?°ÉæwœF?ä:'—Ö?°ÉæwœF?¹L2šTÙ?ž'½(!Ù°?ìÖy¬ÇÒE?ž'½(!Ù°?†ØNÚ/k:?ˆÜÑ-­ØÙ?爛ÄÀ}£?ˆÜÑ-­ØÙ?€¿ÎŽý4"?‹,FŒ?ï½ňñè?‹,FŒ?´@ÄÍA??£z/WAÁ?í}w珓(?£z/WAÁ?`¸É"Ä´?Nè™àº?ïïG6±~#?Nè™àºPSR4FGL J1932.2+2221?æ&zÇ,µý?ùYº`úÀ9ÄN`	UÀ;s'È@½S¸cß#@Hæ=·´?Ó=`]¸Ã?ۉQÐ9¿@M}|,¡I@š@Zãü>?îÑÇ]w)'?ïý¶ÿÛíÒ¿â—DŸí˿刘ö«;¿ïܤ`œøÊ¿ïù¿tµÎPSRPSRPSR J1932+2220?ì."p˜?»ÂöÎí¨(?¼~‹\{<?»ÂöÎí¨(?Ü{nIÎný?ΰ¬_ç?áÂHÛȁ?ΰ¬_ç?è÷În@-?¬(Œ)-E¿?Ì ÆFÿKƒ?¬(Œ)-E¿?आ•Zñ?µËÇöŸ?Þ·ÚòÕJ?µËÇöŸ?Õú tŒf?Äå£[½?åïŹ÷Í?Äå£[½?·fQB½¿¿?‡ÌæU½?í5רH?‡ÌæU½?ÛÝkÎÏ?¹Óê/U¥p?âJþ˜?¹Óê/U¥p?µhϘÌB£?¦¯°kÉûØ?íRæÊúÌ?¦¯°kÉûØMIXED4FGL J1932.3+1916¿ÔœE~lö?µb©ëJÀ7~ÔÈCÑÀ:Ž•yy@•ŠÀÏ6@¬Ÿ€cg®?¨'¼«ë¬?ÛUߛªd@-ïÓh'1@>—û^ۃ?ɍQâ É¿ÐB3µ¿âé¤ÿ~Oç¿èÛӀE4½¿îf«esø¿è*AA¾¼>PSRPSR3FGL J1932.2+1916PSR J1932+1916?;ÝÊ"?@†àê<GÈ?ïü,v*ª?@†àê<GÈ?œ6£ôõ"?ŸàÚ6G×?ïJà<Úì?ŸàÚ6G×?™Üûg@¶<?"éÝWH61?ï1$Ó¸¾?"éÝWH61?mh²z±?µ&2ÍãF?ïÿ4—G•ý?µ&2ÍãF?:¬n½:£ì?-y•ÅA¬D?ïüªrQM?-y•ÅA¬D?j‡Oõøžo?t{<•"H?ïåx°"?t{<•"H?†e*­üÈ«?jèæf"vû?ï¦kUю?jèæf"vû>{w"m­9Ð>€ÚY¥¹¶?ïÿÿÉ=:>€ÚY¥¹¶PSR4FGL J1935.2+2029?ì6{Fi¾,?°¼ÿ¿KôÀ8fpȍ£À:~E܃#6@Ú	Òg@±áYKË°?½(Eëf?ØPø€"Ê«@"³Ïà@{έw?Ôy$ä»ÖÛ¿ØH€aå"Y¿å¬:†
˛¿ì!ùOÖοïÿþÐñ¿ëÈ:a$ÞPSRPSR1FGL J1934.9+2031cPSR J1935+2025?Ú0'9Æ?ÕT{¿
?â÷g·cõ?ÕT{¿
?¶fgH†?·t¼äy?í3,^ï?·t¼äy?Ցv>9^?´×U!P¤â?å7Dàã7Ñ?´×U!P¤â?ËDñ¬U3
?¯TÆ@kªô?é.Ôê³=?¯TÆ@kªô?Ñ3íeÒ{?Ӓf忄?çf	MðC?Ӓf忄?€`i‹ÌK?ˆ»"n¡J?ï¾~Y»÷×?ˆ»"n¡J?ÔÀ.¡Ü'Ä?¸Ûa
Â]?åŸè¯·?¸Ûa
Â]?oš|IûC?^ÛLf'àˆ?ïàeƒÅûU?^ÛLf'àˆPSR4FGL J1939.6+2135?âo'EM£¿ÒÚ
ã]Ý×À8â5~gÀ:Õoê›ë@.|Ì.lO@§ B•¦Æ?¿æ"´4û_?Új{ßI| @°lÊ-¶@Žg£'aï?ï²;†¾Ë'?׈Šþv=¿ã"~aÚ»x¿ç«Œ‹¿îŸ[O7¿ïÿý¡UûŠPSRPSRPSR J1939+2134?tXšÂ)ØÜ?',Ó\Ü?ï×NÊ­&®?',Ó\Ü?¬Ž°ìÎHC?­CÖ¸f—?î7ñžœ?­CÖ¸f—?»×ÇQ¸¯^?¦Õ¡¼æ–F?ì…Èê?¦Õ¡¼æ–F?¦!lŸ+"?Œb×[^/?îé6(ʾ?Œb×[^/?]Å/\×w?}"­=?ïñs†Ž$?}"­=?{φ"É;?‡u¯>"xÆ?ïÈaÀå7þ?‡u¯>"xÆ?ŠÙqŸW™?€¼N
?9ZGR?€¼N
?Jý¶'ë"¿?<à;±]c?ïù@'[%¯?<à;±]cPSR4FGL J1946.5-5402¿»@ˆñ«©gÀ='…¹èÄzÀ9q0ž-}À<§'ÍÍ}Í@-µ"2@5¦à©ùc?°x±'ž‡?âÄ ¾{ü%@(ÐkYnL?ö	¸éžÀ?ìÔ þþ"Z¿Ôÿž[JT¿Ô·ºÁÝZ¿é‰²€ñ,(¿ïÿ«çy÷=¿êO]ë­¹PSRPSR3FGL J1946.4-5403PSR J1946-5403?`¸bÒÉA?jVAšô÷Z?ïïG<U5?jVAšô÷Z?ÅÜÜBSw?ÁÒLÄåÞÓ?êˆÈï{+"?ÁÒLÄåÞÓ?³S-Àns?¡»B2C?핚]±-?¡»B2C?J´•N©Ù?>E·woûb?ïùRÚËñŽ?>E·woûb?•'PòxèP?Àû»5(^w?ïVÅx^zN?Àû»5(^w?¨ñšp/ó ?§Ò·_Œ´W?îpæXÓÅ~?§Ò·_Œ´W?–QtÅWk?‹žêømÏ?ïK…tžt?‹žêømÏ>ÐurÔáæ>Ìqaþ
´?ïÿ÷ÅQ‹ì>Ìqaþ
´
PSR4FGL J1950.6+2416¿Ãþ`KLã¿ò[vH[¹À9Z`,ÃÀ:Ño™\@ˆªFJ@Á¹Þ³?Êuú	?Ðеd¦GÓ@
¸S 8"¬@øᬭÈ{¿êÓà뽩?ïÿ$m'M¿ç`Jù"–-¿çÛ?áíEh¿ïüäW-
¿èü{±QFDPSRpsrPSR J1950+2414?°H!?¤ZŸ—a:j?¤oäû}ö?¤ZŸ—a:j?ÛZƒ…AY"?ηý¬W{+?âR¾=_So?ηý¬W{+?êt¾eMY?­É…æü|R?Æ-jʛ'?­É…æü|R?æ°5IãÎÇ?­<1ÊØtÙ?ҟ•l8br?­<1ÊØtÙ?ä^'k–À»?Ëf†É՘ñ?×BÛ(Ò~Š?Ëf†É՘ñ?­¡»Óµ‡&?·€àu6ë?î%äBà$m?·€àu6ë?×36—Ûm=?»˜¸7dx?äfd´Ia?»˜¸7dx?¸ffrmV?ªGƬ$?ìó31–â?ªGƬ$MIXED4FGL J1952.9+3252?î!?ŸlQ@"™Iè^À6¨V˾°À:¤NA¬rº@G¾"¤9@a59°€?'	ÉSØ?ÑÏrä¤@<¤Y!…Æ?ü°ô9MS›?ꨏ òSo¿Ð"žry¿áÇggî%ã¿å¢l ºŠ«¿íB XÐ{®¿ì†XVÙ+PSRPSR3FGL J1952.9+3253PSR J1952+3252?_üs¢ÉÌó?v?ŒãøÀJ?ïðÆ1ZÊ?v?ŒãøÀJ?'hÈáó´õ?–ÍAßðI?ïl¹¸â£è?–ÍAßðI?¡%~Žðd?˜ÁnjƒæÜ?îí¨Ú?˜ÁnjƒæÜ>eÑ	ùc©>v6…Hjù?ïÿÿéý¿>v6…Hjù?]ìYàg"•?w…Qa¿12?ïñ	ÓŒ?w…Qa¿12?kŸŽ ϹR?yIÀ,DEn?ïä`r«æ?yIÀ,DEn?ƒÌ$Î?jÔ8ÙÓ>?ï°ÏlԐ?jÔ8ÙÓ>=…ˆrôFf=·sEÔ|ù?ð=·sEÔ|ùPSR4FGL J1954.3+2836¿çî˜'Q?×â4½÷ÇÍÀ6òçø¢=­À:{(‹9"†@ODL
D§@‹Ÿ}ß(ð?œC¦·©?Ô¼íÇWæ@4ÉîEÃX°@àp©?ï÷uýÞÄ¿Ì¿¯î¿à²¿-¿åÛibš)¿ìhÄÓTÑ¿ínúSPSRPSR3FGL J1954.2+2836PSR J1954+2836?ARg
t¸t?=ÄI4÷í5?ïû«f9‰¨?=ÄI4÷í5?•Hí0ä?˜ÔÔaÖ/?ïU¿ðÎè9?˜ÔÔaÖ/?†‰Ûüä™R?ˆQ××û{¢?ï¥Ø5¨ë?ˆQ××û{¢>ÞPc¿z§¾>àבA·¿š?ïÿðØ®ê>àבA·¿š?HÔ^Ñ?@Ë×Ïå?ïùùK?@Ë×Ïå?igñ¹ê¿ ?sØ\xj÷?ïæ˜mð¸?sØ\xj÷?'ÀˆXm?W4?3Z?﷈ýêüä?W4?3Z>)¤¤"p¸>:½Kr6ý?ïÿÿþc®â>:½Kr6ýPSR4FGL J1957.6+5033¿ï""mÌ@&	»j¤¹ˆÀ8eŒ«tqÀ;ϽƟŒ"@ýÁ@¸ýé¥K?¨®'zšÇ?威‡ª@5¤A»Œ2©?ý]!ŽpÅ?î݂AŽ?É¿ÌÝÐÀ¢G¿ãµJÐê°¿íP,h=Öû¿îÚG¿ïÿMéDÓPSRPSR3FGL J1957.7+5034PSR J1957+5033?aFn"Ï\Ì?`Ô
øDµ?ï[²ƒ?`Ô
øDµ?¢xRÖÕ?§À20Zý?îØßU³?§À20Zý?®¸"õ^Ê?¡vÎmª¶?îvÀ·ÑÏ?¡vÎmª¶>Ç#Û¶zÓq>ϧVEɬ?ïÿú6Åíh>ϧVEɬ?Y¸‡uFªg?U|£ ÏV?ïó#¼P[k?U|£ ÏV?xoìLpþ9?"£fÄQ ~?ïÏ 'xûû?"£fÄQ ~?Ÿ¥0¯'þÕ? ?pï†?ïÖz†À	? ?pï†>Z?M_mà>3Ÿ.×Qëí?ïÿÿÿv¡>3Ÿ.×QëíPSR4FGL J1958.7+2846¿ïâ6öƒ¡Ø¿ÖÚ
'ºÀ6ùgÉÉãÀ:—"rñ$@üi°ó¨Y@µ€e-?šþËD'?ÙoQ|I|¡@8‡Œ!áÒ?ÿd7È]?ïüÏ^w"œ¿ÄY€ú¼I¿àÁOÁs¿ç]*J¿ì£o÷à¿îBãÈÂýPSRPSR3FGL J1958.6+2845PSR J1958+2846?Bš¤€{|M?=CŽ;iÒõ?ïûYWº2?=CŽ;iÒõ?"5̟é/}?˜ª ¦Hì'?ï^Q›tô?˜ª ¦Hì'?¨5¶&º?ƒÕ&€ÑÛW?ï¹_+ÖêÕ?ƒÕ&€ÑÛW>–s"Üa
>Ÿïû''Û?ïÿÿL%óZ>Ÿïû''Û?QŽä×W?Z•¤»i?ï÷8Ž;íl?Z•¤»i?j¿|+ól?v"
°:š"?ïå@ƒþ§»?v"
°:š"?ƒ%éµñS?gVðǑÆ/?ï³kÀvó?gVðǑÆ/=ÜÙýz³÷Ä>H1¹ÅÝ?ð>H1¹ÅÝPSR4FGL J1959.5+2048¿ì5	ƒó{ÀÄ{gkÀ8Ú·ÿ¶.%À;Àäù}@´šýqÛ:@›ì't¹æ?¯uÝöjÖ?Ü UàÝ%
@%u"BJ'k@•šw?ïÿíUÙPi¿ºÌZ¡Œ,I¿âTI˜ÐEþ¿çIÁ/à˜¿ï-ž§öT¿ðPSRPSR3FGL J1959.5+2047PSR J1959+2048?Z³ã&í]ô?\šÄè)?ïò¦-P?\šÄè)?¥·Ôy0Ç?ª¢µ`ÅH¼?î¯D'ª®"?ª¢µ`ÅH¼?°ê×)'g?¢jA¼³?íâ¥ùwó?¢jA¼³?}žBbÄO?lÀPyqÊ?ïÄÃπ¹×?lÀPyqÊ?\&ïBÄ|?[ïV¡	Ã?ïñýì²ùÆ?[ïV¡	Ã?|¸­1"8?ˆæ-ø´ý»?ïƎ¥}[(?ˆæ-ø´ý»?ž¥¤Âí?œ«‹<°'?ïŠÒßéé?œ«‹<°'?ì»@ßÅ?Z.Eb?ïÿg8jÌõ?Z.EbPSR4FGL J2006.2+3102?í^z£y¿á<Âþí±IÀ9?ô³›£_À;p.fDØ@ëÏtœ@¬¬Ñ"Âr?Á¡Èg7r?ÚÁl!'J@×Aü#Ò?Ý#Š'ÇpË¿ïþ2Œã(?ïòX½[jµ¿ßՁ;ÔÂe¿å+ùæ/t¿í"XŽÛP¿ðPSRPSRPSR J2006+3102?œ(–ª¯t*?³ý2ɕ†?ï»Jª"_?³ý2ɕ†?­#î«E×?±pÅ-ÿ¿)?î-Á"jÓ?±pÅ-ÿ¿)?Ça››§eà?­Âƒù˜^?ê'™&ˆ?­Âƒù˜^?w3†i?a6ìߒ{[?ïјòæÎ?a6ìߒ{[?Œq"¼7µ?·?BçÚdþ?9ú͑?·?BçÚdþ?æYÃò.ð?wkÌuǪ?ï¸f™3"?wkÌuǪ? ¾¨jïl?•û{¥¬'2?îþDP¹?•û{¥¬'2?½IÄÞ9®?	\:›û¯?ïÿZu21?	\:›û¯PSR4FGL J2006.4+0147?êd'‡žÀ/ŒgœÇK"À:ŠsùÍÀ<¬é\OŒ/@Š"Yé«U?ÿ4?Žò?ědŸç¼g?Ú·u¢™r'@ª•…7âÅ?ï‹x~™?ïÊ\ô‰?·ºä—ï ¿ÍÂ\ÜNõÜ¿Ú¨ÓÞ¹ß4¿êÓÜ¡@B¿æg€)ÙîPSRPSR3FGL J2006.6+0150PSR J2006+0148?اÜL
‰`?Ð?`Š{¼?ã¬Ùú»P?Ð?`Š{¼?É
°) Z?Åï'_?é¹ýSõ—ê?Åï'_?ã½ÿ»¶›?³WæBì?؄ˆÄ'Ê?³WæBì?üL%aRD?£ec8ø/?ëìö§«o?£ec8ø/?±!"y:?·ÏŸ'±)?íÛßOcóù?·ÏŸ'±)?¢'ÛøDçê?¬|Ïï£Ò?î×Ò@mó?¬|Ïï£Ò?É%HEáX?³T CJæ?鶭ú?³T CJæ?Š—>¬€TŽ?{¡õSkÇU?[½?{¡õSkÇUMIXED4FGL J2017.4+0602¿²{éw=Ô@À0Ÿb0vÀÀ8dÝÐ*OÀ;˜Å~ð¡@Ùtæ[ê?úក‰'\?¤ŽÁ¬æ±?ÚDãÿï9@5­¥¹bŒ½@/j¦¼î?ïÔ°á´»^¿ÁAá_¿ÌëõF";¿Ý¶0©7 ¿ëŠ÷0ÇÉ¿ðPSRPSR3FGL J2017.3+0602PSR J2017+0603?d0|…ц?múuųŒ¸?ïëσ­Áf?múuųŒ¸?¤ga×ï\?ª6ÈY™¦?âJ+?ª6ÈY™¦?² Ï.V§?£
J¢3Ⱥ?í«æP¹+?£
J¢3Ⱥ>òì¬6ڀ>÷©Óf-^Ú?ïÿÚ&ÄŠ>÷©Óf-^Ú?]ØrDX†?R²džì÷?ïñp"™'ü?R²džì÷?}LºQú»t?ˆVí5Ò?ïÅf‹œ£1?ˆVí5Ò?™X•š®?"ÊcÎÌûH?ï5?7­°?"ÊcÎÌûH>Wú…å¼8>'ä‡Ï–Ø´?ïÿÿô0WÐ>'ä‡Ï–Ø´PSR4FGL J2017.7-1612¿ã<]©ÜæSÀ:4ÕÇGQÎÀ9ÎTæâ!ÉÀ<W^Æ^ô'@ˆ*Û Ð@䲁Çë¼?¸	{>d¿?ÑS•ÿ0LN@»Ÿ'x@mK–¬T\?ïê9>åîݿݒK|U;¿Ø¶<?@ˆ¿â•V©Zý¿íÂû'²ö¿änÒ ÷0ùPSRPSR3FGL J2017.6-1616PSR J2017-1614?ßé—Í€j¸?ɁOý)?à4?ʤ?ɁOý)?ãÿâ*ðo?˗œ|«Ô?Ø;ߪ#?˗œ|«Ô?äïjÓÕÍ?³Î«¦	à?×Ø!*XTf?³Î«¦	à?âe'¤›¼p?­Ó%uh3†?Û4ú¶È‡ ?­Ó%uh3†?›û}8?˜{Ê<(ï?ï 'Ô@š¶?˜{Ê<(ï?ÀJ n¤<O?ÅOræÉÅ~?ëíwäVðì?ÅOræÉÅ~?·mkJO)?¤˜í³]v9?íRŽñk?¤˜í³]v9?¼L´,j?¤ïWŠW;¹?ìv|É:s?¤ïWŠW;¹MIXED4FGL J2017.9+3625?äb1_7aÛ?Øç;x| À7`C{ÓÀ:l«,i—@Þ$ªÚ3¾@ªY:-ù8?¦ÐNƒèú¢?á߁ëR@1í_‹Î@¨¹(«?j•ExZ/¿ÚlªMF¿àPhb¿è¹¿èîú‰žyÓ¿ï4ör2M¿é"—VÉ:qPSRPSR3FGL J2017.9+3627PSR J2017+3625?YîQNð?]À¥lΚ?ïó×{7À?]À¥lΚ?›Œ«õfÉä?‡üŸ^À?ï#š ?‡üŸ^À?¢[Ð_yCU?™^õmz¸Ë?îÚBùú­[?™^õmz¸Ë?¨šÄ"é?…ÈS|H?ïÿ¥]ƒO?…ÈS|H?BÚ"­#…?5
!‡¢ã?ïûIwmIÚ?5
!‡¢ã?ru‹™8A?}§?M¶Î?ïÛèç¬ï?}§?M¶Î?‰;ÔëŸãÅ?zšNAã?lýQ?zšNAã>]j¹µ|S<>bD—áWy?ïÿÿñ%ô>bD—áWyPSR4FGL J2021.1+3651?ï‹Õg'?»ì˜ïû{À5^Ê÷àÀ9¿-<y-@îý­•O@âXýÈ[?…\¼!6?Ձòžm"×@J^$_ZÙj?ý|$C?ÞÔûD"i\¿Ða1ޟ](¿áLà«üÉ¿æW~6fÄZ¿íZhµËÿ¿îqžBuÆPSRPSR3FGL J2021.1+3651PSR J2021+3651?[X‹nŸü"?d 2Nn²?ïòSº<Qj?d 2Nn²?'C-QFï~?™*ø¸ICQ?ïu敺€´?™*ø¸ICQ?ãM.<lƒ?^pkªum?ï¸r˂'–?^pkªum= ´Wø§/h==J/?ð==J//äΙ?pÜE[ËQ?­~gØ	•?ïÞGu¬ÌÊ?­~gØ	•?b6"‹rÅ?qüŸr~|?ïíûÉ9šV?qüŸr~|?'WZds"?XºäÔhÀ
?ﶢ–˜]Y?XºäÔhÀ
?ðPSR4FGL J2021.5+4026¿îuø#V‹@§~¼ž`À4æe×Ë-À9E¼Çœd@̧"W`9@èEc·_}?‰ñЁ&?Ù~†TB@Lôów[0@nÇ­Ô¿Ñ&s1P¿¸{w€Ñ1ò¿áÉ^ƒCÿ¿èU±|æ¿îÔvå9«¿îõ_þmXÉPSRPSR3FGL J2021.5+4026PSR J2021+4026?ç»áÊñ½?η3"«C?Ј=új‡?η3"«C?X¡hU¢?"Ó•Ö`Œ?zFz?"Ó•Ö`Œ?Ցޕ™|?²í»L$y?å7sµ3B?²í»L$y=W6q^ïßM=xùmœžl?ð=xùmœžl?áê@¾¿¡t?Ëlàv¼d?Ü+~'€½?Ëlàv¼d?dµºëX"?rîƒ=Óm?ïëJEh]?rîƒ=Óm?á_Ɨ²?µQÚ¾'?Ýõ@rЛÓ?µQÚ¾'?ðMIXED4FGL J2022.3+3840?¼UP©æ˜Ñ?î=oâ'JÀ8tPrßÀ:‰ƒùdo@8'l+w@i_?*¸?¾—R£/š?Ú8ªkxõ@©×ý'w>@,Á®
¿Í?îZná_+	¿â}]"ðÅпèrçÉ0`¿ç¹" ]îs¿ïÿë<ú\R?ïü›¦2ÚPSRPSR3FGL J2022.2+3840PSR J2022+3842?'yꉪ? ÕG'P4?ïl0¯—ª#? ÕG'P4?¾Çz½áLŒ?»ÿ}õµ_"?ì'¨CÖo?»ÿ}õµ_"?×øàHõ?¶À¶b–çÒ?äõÛø?¶À¶b–çÒ?ÀˇQ¡?¦.8~ã—?ëÍ?+—¼?¦.8~ã—?–߁±û£?³ë ‰ E]?ïIò}áW?³ë ‰ E]?‹#ïéõa?"ë\‰´Ô?ï"÷p[Õ
?"ë\‰´Ô?ÊuGôj²?³K–©pŒ?éb®ÂåT?³K–©pŒ?YöŠpéÅ?Põ·½|f?ïóº­n?Põ·½|fPSR4FGL J2028.3+3331¿ÜÞÒŒâÀ¤‡3eˆÀ7™ìløÀ;7ý˜F³@ļ YÒ@'ågÎE?¢1R»í4)?䪘Å^C'@8c^t)ž@úúr!…Œ¿è0SðBÛ?ÓÆìM›"F¿ÔôÃ@±öÞ¿çâP¢Yܕ¿î9Pƒ¦N¿ïÿþÞ÷PSRPSR3FGL J2028.3+3332PSR J2028+3332?DÒ/§08?JÚ{í ?ïúù˳r3?JÚ{í ?—Ó½ó9IØ?›T›+͵Á?ïAbsô!?›T›+͵Á?—¨ßOæS?'úò.n?ïB¹£5­?'úò.n>¡ä¼LzV>¦òaXoÚÆ?ïÿþáÙ	­>¦òaXoÚÆ?@(j‰Ÿ?8ƒ¯5ƒã®?ïûõå}{^?8ƒ¯5ƒã®?kÔµ,ÔÀ¨?tïD¯Ôå?ïä+KeO?tïD¯Ôå?ƒÑ¦ð…?eâ
²f?ï°¹dv]f?eâ
²f=Ò*¯ e=é¶Aï‹F?ð=é¶Aï‹FPSR4FGL J2030.0+3641?çò¸áªÌ¿¿÷ ²BÀ7ìºç£À;EWøåZ@ÖâVÌÀc@Mø±W%?­Fk\?ãÛ'8S-¤@1-û¹@ÂC*8ä¿ïsÎ>º?ïþñ­VåÀ¿Ò@묋å¿å)µ/ê©¿íñ™ O–@¿ïÿý`éNäPSRPSR3FGL J2030.0+3642PSR J2030+3641?AC™Ñ ?E•l•ûÁ?ïû /
º?E•l•ûÁ? ¯{0·}¼?¢˜~J4‹á?îõM+ä?¢˜~J4‹á?"ðá´Mk?t\ùI:X?ï_Èx»cÕ?t\ùI:X?ÃkE¨‡?À¿`5ö?ïÿ òSo?À¿`5ö?McØÏ/ï¯?JBg»Á¨ø?ïø§
	]?JBg»Á¨ø?pcöÕü?x©©!°W?ïß8|?¨?x©©!°W?†Éߐ&‡?x¶Û=ÂÕ?笠ØÆw–?x¶Û=ÂÕ>pw¡E÷~>u…w'Œ)5?ïÿÿß@9M>u…w'Œ)5PSR4FGL J2030.9+4416?é1?Й@%z
XÀ7ßÉÇ^ÏÀ;(öýø¾Ã@Vv&LðÊ@Y ¡`7?ª'ýÀ'%?å-‡ÂÁ@0¨…<ƒE?û#H÷ë‰{¿Õ!ΜZ¿¿Õ{½ZéÛ{¿Ûúd_¦¿êŒY?¿ïùºá辿ïqÊG·N¶PSRPSR3FGL J2030.8+4416PSR J2030+4415?C\+ó?I" "¶4?ïû(Ü(pž?I" "¶4?¡Ò§Iˆô¬?£?\q¦þŠ?îâՋžju?£?\q¦þŠ?'=
ß1?ŒN v4ç?ïoN¡B—?ŒN v4ç>ïHk"ŒC>꣯ª"?ïÿà¸'ì>꣯ª"?=äî_ü5?2þ,ú2®M?ïü_ã{¡?2þ,ú2®M?vµ•U>¯>?~WR<«?ïҔÕd é?~WR<«?ƒí;FÅé±?e‰›ÿ3T&?ï°Kç¨	?e‰›ÿ3T&>Kóá°ó>Yb ^o¬?ïÿÿùK*>Yb ^o¬PSR4FGL J2032.2+4127?¾Sòà «`?ðbá& %9À6ªŽÊ2¾™À:U»¹@ßuÚ!Ê?ÿ· ÈÍcÌ?žYÊC'?ØÄ6Ûß9a@7ÎáXu@7M­ÝÉI?èµólsÆ¡?££ä¡)ÛÇ¿ÕP<ÙO<¿àR©»OÌÇ¿ë†=Á×{R¿íIš³uòPSRPSR3FGL J2032.2+4126PSR J2032+4127?Ž:!Y+?¡™¾}_Äd?ï{Ž/z?¡™¾}_Äd?›0T,
þ?DäðáÓ:?ï&}[†Ÿ¨?DäðáÓ:?®Ÿ.ƒöð?¡Ó]œ©ž"?î
Àÿ?¡Ó]œ©ž">ɒ4(:Fp>ÏÝhçr‰Ü?ïÿù›žà>ÏÝhçr‰Ü?nä#1†«m?lÛ¤Z'¢p?ïáܲüu?lÛ¤Z'¢p?oeŸxÍ‹?xIwÞnÅ?ïàš`­®"?xIwÞnÅ?§N™¨ù'?œßF½wÇ?î‹e‹ä¿?œßF½wÇ>?A¨;>>%}h'Ë¿î?ïÿÿÿv¡>%}h'Ë¿îPSR4FGL J2035.0+3632?×BðØEðÀ»K›	bÀ9 ¨,"	À;Ý©Çå@'L
QÍ?þ°ð˜ƒïä?¹§µ\˜²?ê€ÖõD»@(WšÏú@ˆA¿ïÀ‡—ů?ïÿ胸›?¶Øíþ†êQ¿ÙÒ¾éµ:à¿í™pŽR>¿ïî$ïßvPSRpsr3FGL J2035.0+3634PSR J2034+3632?`%J‡û›ô?kÐÑzl¾Ö?ïïÚµ\‡"?kÐÑzl¾Ö?¥º¶‰dN?§pfλñ?î§T‰«K?§pfλñ?¯¢(©)u? ‹XGÇ?îÝuD-_? ‹XGÇ?Sg[Õ¥û³?EC-d¹†/?ïöLQߓ?EC-d¹†/?Z7 Ý€?\ "…ƺ?ïòä/ƒÀ?\ "…ƺ?w¤RÏžÔ?"4GBÿ?ü?ïзZŸ³º?"4GBÿ?ü?²Íüž\Þ?§¸	Esޑ?í¦@l4d>?§¸	Esޑ>ì*hË+¥é>åR-o«&?ïÿãÕÒÚÙ>åR-o«&PSR4FGL J2039.4-3616?ïóûuŠNVÀBEò×sÀ:`
ôGÀ<œ£äv6¾@­ùÄ|œ3@Ží¥,u?ÀX[
è'N?Ù©íœ@(R. ý@–ÖÇL…?À×½ìŠ,¿ãˆÄvW˿ڟ[O7¿èŸ5_ˆPÇ¿ïþ£ßm¹A¿ï§匷3PSRPSR3FGL J2038.8-3613PSR J2039-3616?êp8s)?Âvøb…cà?Æ?ú3YÁ?Âvøb…cà?îââ\£f?¨¹?¡Þ±×¢?¨¹?è¯$âÓ?®CÅ#KŽ¾?ÍClwˆ³Ô?®CÅ#KŽ¾?ì`˜M¶Ž"?›ëÒx<ºŒ?¼û='K‹^?›ëÒx<ºŒ?×ýÎêUÁ?ËÊE
K3?äŠÕp?ËÊE
K3?ç#+©&?ÐÈY¢«£?Ñãù¨­´?ÐÈY¢«£?֙wV"Ì?¾@RoRb?ä³vDTîš?¾@RoRb?à©*ÿ1£?¹e	¿ehâ?Þ­ªñœ»?¹e	¿ehâMIXED4FGL J2039.5-5617¿Ù9ªèî¸ÒÀB'ÁDŽPÀ8êÀ<Èe^ÿj@rŸÚ¦T?ÿ©D1ˆ8?©Ólà9Lc?ÎSíèÑ:E@#_'`4@6Öd¦à¿ØE2¤—ú]¿ÞÏ|_LØ¿Ýhã«5£¿âfB
f‹¿ííC/)¹7¿ïÿùëñPSRPSR3FGL J2039.6-5618PSR J2039-5617?Í0ÑÊɤ?ÁÓÆ!s(}?è³û‹M—?ÁÓÆ!s(}?Óדװ"?Èj«Ø¾ü?æ6'îö?Èj«Ø¾ü?ډtkjdÖ?²Ú¥ÃŽY?â»EÊJ͕?²Ú¥ÃŽY?à¡ÁfVê?¾š¶‡"?Þ¼}3ÝR+?¾š¶‡"?š®fÐ܋c?—÷–ݤ á?ï*ŒÉ°e?—÷–ݤ á?´!¬ÌG?¶n_[¿ =?í{Êf@%à?¶n_[¿ =?Æ»Ð-ÝçZ?´Ù°
fó?êQôˆ†*?´Ù°
fó? 
eíAL×?'_¢L҈Ò?îÿY ôñs?'_¢L҈ÒMIXED4FGL J2042.2+0245?қ¦ïÃqÚÀ7	üȽÀ9Ù©?ÿÊPÀ<QÙŽuy@ðªÏ÷Ð@x½ì_9K?¾­odfÜÙ?ä"_¾+Ÿ@@ »'-ºMn@¥P<³?ïÿÿ^ðP`¿×QN¼¦Žõ¿áš'ç°ë¿ìúE`²Ge¿ïþú¡Ç:'¿ê–­ÁnʹPSRPSR3FGL J2042.1+0247PSR J2042+0246?ó	¼06B?£#ñ0`CW?ïˆ3ÙS÷W?£#ñ0`CW?½`Sk¦°ó?½ubW¸ú?ìSõ'‹)â?½ubW¸ú?Å>¯"Óü?«sØ8ž¡?ê°OT7K?«sØ8ž¡?–JZ«Âò÷?A.3"ÿ?ïM­*x­?A.3"ÿ?–)¨è8…z?ºGƬæí#?ïN²¹ô?ºGƬæí#?•'÷Y€^f?›lI
ìÐï?ïSpEjöÍ?›lI
ìÐï?²Êùå"?¢aŸ?;xS?í¿¦ µ?¢aŸ?;xS?9IŽ8ˆ½,?*Ç7õ¢?ïüÖÎ6	?*Ç7õ¢PSR4FGL J2043.3+1711?ãvòôþ­À.¢(D€cÀ8H…'òQÀ;½·ý1ïf@f­ZÁ—?ýÿ´€¥¬Í?¢sz ,›??Ó<ëƒFF
@0©:÷LÓ@Ú>›ò{?ïÿؒӬ»¿Ó³ÚøßzN¿Ù Ú@'ãI¿âŸ>HÀc¿ëò¬MÑD¿ïÿÿ)@k*PSRPSR3FGL J2043.2+1711PSR J2043+1711?uÄ[ðYÚh?x…¦,'õ}?ïÔwHo"?x…¦,'õ}?¬€£ìhOs?°{Êæýd?î7õÁþ)?°{Êæýd?¤÷­jâ?›žšºté3?ERš'?›žšºté3?B!†§ÊR?@8ìö¯ê?ïûw¼hë@?@8ìö¯ê?p¶a"r,V?jÌ'%B?ïޓ=b8?jÌ'%B?‡ž8‡'t?ZY
ÕY?‡ãb?ZY
ÕY?'ÎÆY|?"7£Ã.·z?ïq‰ÏÄpT?"7£Ã.·z>À:…œ¸>Çq';'†?ïÿûþ"™O>Çq';'†PSR4FGL J2043.7+2741?°A©ìÃ¥@À"Jeà.©aÀ9sZôB\œÀ<%ê°¢¦@õ'¦¸'@+e˜U?¶'«hÎös?áëaŠ@ ö²(ܘ@ÆÞ	àÿ¿§˜»"Ujk¿Ðg°Ql¿ái¬}Ãû¿ì¬#ßÙ¿ïÔ÷©i^¿ïÕ@¿ð©PSRPSR3FGL J2043.8+2741PSR J2043+2740?æM
…ü?Ô7‡©Š°ü?Óeêô×Ã?Ô7‡©Š°ü?Å]x¬;?ò=xãR?ê¸h¡Ôüq?ò=xãR?фk€'É?²lõxqé˜?ç=þJ?¶œ?²lõxqé˜?Ô#šÞVü«?±G³®ÿÄ?åî2Ô«?±G³®ÿÄ?¶™Š¼^±?»8Óí8¹@?í,ξzµº?»8Óí8¹@?œáæ9…\Ì?¨*™aö?ïðÍïê?¨*™aö?ÕRªw7o?·€žÀ›?åVªÄdH?·€žÀ›?‹&R"o+€?u~;‹k3?ï"fµÒÆr?u~;‹k3MIXED4FGL J2045.9-6835?éÇðôRÀA»>ÄaÀ:âØK%À<ö¥Nفç@ßé"ÃÏM?ü<cþ­©?Ë×î©ksÁ?èô¨H‰Î@uh¿ÜúA@"…£Ãi!?­t²ÄL¿àÞç+ž¿Àøÿ%:¿ãz›#¿îR£`—ÅY¿ïêÈ@ +šPSRpsr3FGL J2045.6-6838PSR J2045-68?º|,¿YOZ?Âþoµ€¼?ì°zhÖ?Âþoµ€¼?åQ{âhYJ?ÊìՑÿ?Õ];/Mm?ÊìՑÿ?ÕvŒ± @_?²í bJK?åD¹§oßÑ?²í bJK?ä^"4wMa?²5²·1`ô?×Bחe>?²5²·1`ô?Â_Ë2ªŒ?͒ô)ï"ô?ëh
3U~?͒ô)ï"ô?Êjµ¢E?Ë=črB?ée|—~¯?Ë=črB?Ä1t$F?®EÁÄÅ°?êús¢þ¶ï?®EÁÄÅ°?ÃTÍ.=ø?®è–ú$k<?ë9êÌ´p'?®è–ú$k<MIXED4FGL J2047.3+1051?ì¹"Æ,0À3º­æW¸NÀ:K¼£n/À<8öí1Ç"@Tö.šó?û4+'»?Á†}]"ñ?ØθêÑÆ@£'üÇf[@¹ù$¹	¿îü¶¿š4I?½_e@KŸ'¿ÖEìuæ¿Û
b¿ù¿ëLóc9‹<¿å€Þý{ì5PSRPSR3FGL J2047.1+1054PSR J2047+1053?î¹$ñ«²?¦²xьŸí?¤m¾CxùÝ?¦²xьŸí?ïV`?Áó? DàÒå«ñ?•3øâf? DàÒå«ñ?êWS×v'?¯°	ôO¼?ž¢°¢'e?¯°	ôO¼?ï h¤Èæ}?{W—ÐóvO?›òëfã0^?{W—ÐóvO?åߨeJ˜¼?É6sHeä$?Ô@¯5jΉ?É6sHeä$?ëBPGž­³?Å4¹}2l?Âö¾á…I3?Å4¹}2l?×	+úÒ%?¼OFlÔr;?ä{j–÷í?¼OFlÔr;?ìttÀžw?¤ôqVˆ?¼\YÿóI?¤ôqVˆMIXED4FGL J2051.0-0826?­½Š™À>cC,¥zÀ:š~dž;ïÀ<¿,Áÿê1@›™¡ýj@o	A=?Ä©h?ä¬(²¦°Ù@Ñ'o°'?ü÷WØYý¿ïÿøþÙå9?ïÿ¼]éÀ#¿ÊöˆÝߙ®¿áaÝøï¿ïÿÏ"èbU?ïõw`‰­"PSRPSR3FGL J2051.3-0828PSR J2051-0827?ÃX
åم?čºËþî?ë)ýF‰žœ?čºËþî?Úâ4éýÆP?Ì⧕ßc?âŽå‹Ø?Ì⧕ßc?Ö#:Ko-ú?±à*ÜÿH?äîbÚHi?±à*ÜÿH?Úè#æö)ú?´ÅÌ7݄.?â‹î"ë?´ÅÌ7݄.?™gµ¡#
?¢'4L]³?ï4ÂR܂?¢'4L]³?®PÌ†ÖÉ?µRýzR?î÷#|JÃ?µRýzR?´õ—™ª¯˜?£¬mþ''(?íaM
£Í?£¬mþ''(?¢"'±Ò?"yP€PÑ?îÖ½‡Æ™"?"yP€PÑPSR4FGL J2052.7+1218¿ë·ÄaÀ3ýµc#»ÇÀ9äÂa8ÿüÀ<(2áԛÎ@>"«n@8Ÿƒ¾f?½–^%Ð;?ÃB'_ŽZ÷@ûšþôg@à?¸o?ﱿàÖ'¿án'xbè-¿âÝ6;ü/'¿æÓ\.§¿è0dxO¿ïíh]â^YPSRPSR3FGL J2052.7+1217PSR J2052+1218?ïîhš§ƒ?^'p.zŠŠ?a—b6Í8?^'p.zŠŠ?ïbèúCÂ;?žû
ù¸{?"¢à°¨€?žû
ù¸{?ïÊ(4Òo¤?{,Ãñɔ?zëåèö?{,Ãñɔ?î)ßz#ˆ?‹ÕUšVÑö?­nbî+‹?‹ÕUšVÑö?îü!f,/?š\pKöU? 7-íèÀ?š\pKöU?ì¤J+a"?¼Œóe_L¹?ºÝ®¤÷#k?¼Œóe_L¹?m,˜?XłÅ[ƒ?¦þ4½š…?XłÅ[ƒ?çp咸Ì1?«KÂÜj÷?Ñ4ڎgž?«KÂÜj÷AGN4FGL J2055.8+2540¿‡ÐöDm×ÅÀ)
7.jwÀ7ªÃvõØÀ;¨ÿ°NçÅ@KüŽ0"Ø?ýpä8ú'?ž:öËù¾?âËt8Ùe@Al?Ä;.@ñœs)˜?ߓ~AÏXB¿«,F¯çº¿ÜÉ¥%	ó¿ê "àwN–¿ï z"Ԙ¿ïÿ atd+PSRPSR3FGL J2055.8+2539PSR J2055+2539?'ìÌ·H?+?–š#Ñp×?ï´LÍ&þ‹?–š#Ñp×?˜xø?ŸC"5xô
?ï?8ƒ»G?ŸC"5xô
?—mú̒ÔÔ?Ï7'á?ïD)r.
?Ï7'á>8X,>NŒO7R"Ö?ïÿÿüÇ]Ä>NŒO7R"Ö?kðtKD®?Ÿöñ'càê?ïä‹°š4?Ÿöñ'càê?pš1	¹B?€°Xpá?ïÞËѾèÍ?€°Xpá?ˆÙÛ(/I?{¿ƒðYS·?"£û?{¿ƒðYS·=D͜Zj ü=y"î6kP?ð=y"î9'ÿqPSR4FGL J2111.4+4606?îÛÊõé¿÷Dº)\ÜÀ7Ä 
a'ÒÀ;Zƒ®Ò@iÚקqI@#.£yè?ž¨e—çñI?а.[ˆ@,Q¾ôœõo@qÁcb%?ïÿ–¹‰$¿Í}÷<7ç¿àø¦Ú'Q¿ã@5z5PD¿ì¹Fk¿î<@".þñPSRPSR3FGL J2111.4+4605PSR J2111+4606?z ÃÙÚä?"º'pÚä?ïË¿[o'?"º'pÚä?¥™ÓK"/ƒ?¦…|‹?ß?î¦b˄ÖÈ?¦…|‹?ß?½«ŠƒNï?§ïkƒíÆÿ?ìJŽ¯ŽV"?§ïkƒíÆÿ?Bk"ƒ§\?:±²øì"^?ïûe›T7?:±²øì"^?{aOÕ™?£Êm}ÛÖ?ïÉ=aƽ?£Êm}ÛÖ?yýú"§'X?'àœÂŽ?ïÌ8©{?'àœÂŽ?'ÅHÒ?ŽŽ§®¿¢?ïoïaÕ»'?ŽŽ§®¿¢>Ã%=]Lÿ>ÇH»ÕrBÚ?ïÿû8x >ÇH»ÕrBÚPSR4FGL J2115.1+5449?æfùѽ¢b@{>—ÔÀ9«Ã½Y'CÀ<H:vôS$@ AjT‡–¸@S%A(Ï?ÀÞjÄoF?éyvCS;ç@ Yªu[Í@5euû…¿ä'pÀ²b=¿ßò([¾Âž¿j‹éÐ
;e¿Ü=eü‰(¿ìòª¬çT8¿ïÿÖ"î9PSRPSR3FGL J2114.9+5448PSR J2115+5448?
¤GPI?¬ûu[ë›ì?ïÁê·™Ï?¬ûu[ë›ì?´»hM%µ?¶#ïcôž?íh'ö'C?¶#ïcôž?·ÞԑÉ2è?£w"[h"?í%mðó?£w"[h"?‹¡¯	9Üè?s.¯0ÕÃë?ï'yCÛŒ?s.¯0ÕÃë?˜•ê¨ùàŒ?ÂÒFò‹Uè?ï;Pª7<?ÂÒFò‹Uè?‹ÕwJ¢+2?"-[ C?"¹ús?"-[ C? MëІa?"¡'Ç0X?îû!CŠ?"¡'Ç0X?2zDBŗ??&¶=¡2?ïý°·dÓ?&¶=¡2PSR4FGL J2124.7-3358¿±•2BI0ÀF¸øa¦
EÀ7ú=ú	FÀ;Óc7ݼß@꓇0á?ùp0dKÙó?¡¥€­oÊ?àÿ‰kV@=÷Ú+Z!@)‹ê"n?ì0`†R•?Ĭ	É,"B¿ÐÆÚ¯ä^º¿ä>÷âz3"¿ï"NB_Ì¿ä±ÈcäPSRPSR3FGL J2124.7-3358PSR J2124-3358?'p·?u?±*̊YK%?ï{tQ
µ?±*̊YK%?¼×GÏÁ|?Ådb0²áz?ìeÆÐ?Ådb0²áz?®i 1Ø"?ŸaøÍĊ?îéeÅè¾?ŸaøÍĊ>x!jÖk>Švž'†÷H?ïÿÿÏ%$>Švž'†÷H?—» vëF?À>EtË?ïB&ü>æ?À>EtË?"ÈQà>æè?£1}¨?ïY½qBÀø?£1}¨?­"/Žd¼€?©d}ŸfWæ?î-Ýðxè?©d}ŸfWæ=§p¨JßZÜ=Ø̕Žýڒ?ð=Ø̕ŽýڒPSR4FGL J2129.8-0428?Î*¯ùNØMÀBz弇Û+À9»†ýX†À<WêpKÂ@PV¤&c?üûtëdg‰?¸+ƒ–%F?ÝN-?SR
@ 4)ˆ;£@)nÑnòý?ïøï]€¿²ê†qÏt¿×Â??°ï÷¿å•yyh¢¿ë·ù1~'¿ðPSRPSR3FGL J2129.6-0427PSR J2129-0429?"ðŽèç?¥ip"{É?ï`{‹¿Á?¥ip"{É?Çb?Bé'3?ÁÃÒ8'¹"?ê'p/E›s?ÁÃÒ8'¹"?À£ð?m©&?¬.9"†HÌ?ë×ð$•·?¬.9"†HÌ?¿ƒÀ©ÓÎt?¥J®u¯ë§?ì‡êņ2?¥J®u¯ë§?e|¬{W?hXMAyär?ïêïƒlAÙ?hXMAyär?¢Z»sš<¾?¡÷ù¯Û"³?îÚTHÆ\4?¡÷ù¯Û"³?"¤' ²%w?ŠüËÐq'?ïbÞÆì°d?ŠüËÐq'?{Æøbô?pQ° »?ïÈr#õº?pQ° »PSR4FGL J2140.0+4716¿¢‹y~ÉPÀÌ~É3»À8X«m×sðÀ;ÈY±L=Æ@3xÁ1ãþ@}`ݐi?¨Gq¿Ç?ä¹V}»Â@2fz–¼?ûÃrƒU4¿ÐË+!–Ó—¿À¯HW‡¦R¿à}·³àm¿ëSž­ÕÁ¿ïÿr;†¾Ì¿ïÿ÷Âé±PSRPSR3FGL J2140.0+4715PSR J2139+4716?WþI¥0?_ld¬ÐÍ?ïôÚ軸?_ld¬ÐÍ?£RË'yõ?¥,0Nk6Ê?îÊÓN'UA?¥,0Nk6Ê?™@N¡\?'0‰
D ?ï5ý&<ï?'0‰
D >çžìÚ4l>æ_xCdÁU?ïÿèa9*>æ_xCdÁU?Uh!í/¬¸?pË¢Gîw1?ïõKïAÁÁ?pË¢Gîw1?uú½\¥W?OI§†qÀ?ïÔ
…XÞ­?OI§†qÀ?†ÈUåQãS?qb§"ÖÚ?ï¤Þ¨†5S?qb§"ÖÚ>:"Ÿ!i0>A}ö֎û.?ïÿÿüÇ]Ä>A}ö֎û.PSR4FGL J2205.5+6016¿ïö]?îz@
è<v©À:zD& }¹À;¼š*¹@"5ÜP£@¾mþ
?Þ
üÂÞ·[?ïýÖZHŒ@¹'m-*@äBtä¿ïÿÞ°ô)?ïÿó5bB¿ÞEÿÉú5¿â…¾'bE¿éû/¶¦ñ¿ëù¦_$ӟPSRPSRPSR J2205+6012?îG™;Œ?°Ã¯m-a?«Žöi³ŠÍ?°Ã¯m-a?퇽ž(?¹&C6"¶??³ÂwM?¹&C6"¶??ì<‹¨·'?¦n£ô&Þ?¾¢ºCw?¦n£ô&Þ?è3…§ãøý?²[‹³¾8(?Ï1é`p?²[‹³¾8(?â.bè=Ò°?ÍB½[X?Û£:/"Z¡?ÍB½[X?ègìÁðáæ?ÐÁ`-ÎUŸ?Î`Lø<xh?ÐÁ`-ÎUŸ?è4ÐÀˆ'?²–sN2;\?Ï,¼ýÝ÷ÿ?²–sN2;\?ÐåŽbŒoÃ?º£"o8G?ç8ιÈ?º£"o8GMIXED4FGL J2208.1+4058¿­øí‹51À(/ëkôDáÀ:ÚøßzNÀ;÷։1@éÏç3€`@=r6~AN?Í&¢+8'ï?èÜsÔ
2î@
ç-@™Á1¹?èQpjÌ&µ¿ØTfB
g¿ì|º–¿åù`ß=虿8ˆÊ¿ïÿ5À+SÁPSRPSRPSR J2208+4056?ï
Øe3?¤ŸqIï7[?ž\…«'–?¤ŸqIï7[?éœ;"¶?É8zX''?ˑ³å(?É8zX''?ì£âkù?£y6<qH?ºäì 8?£y6<qH?ã播äv¯?³6©__a?Ø2Ú¤7¢?³6©__a?íùpx[?µ¤'6L8?°7¼}ˆç§?µ¤'6L8?Ði6¹Ý?Ñp–òN?çËtäó#?Ñp–òN?ågç‹G¤ã?¶ÁzŠ?Õ00ép¶:?¶ÁzŠ?°ÓV<¢ž?—!–¬º?íåŒTó³}?—!–¬ºMIXED4FGL J2214.6+3000?ܨ&güF@À5¬9-Œ*À8)"UUÀ;Þ\Nµo¹@û—OgqS?úð.½§?£U$'ìG?ßmrÿÑÜ×@9ÔfõŸ@§]žk»?Ó˜ÂÚÄ¿»ã3–…h	¿Ö\²3¿äʵ€í ¿ïÿéYËMq¿ðPSRPSR3FGL J2214.6+3000PSR J2214+3000?Ž2	•?'<8$¨	?ï‡ï7°Æ\?'<8$¨	?«‡À2|¡?±.gjÃY?îGƒüñ¥?±.gjÃY?¦5'×/<´?šÂ<1´ƒ?Қʥ?šÂ<1´ƒ>Ï-f°S>ÔÚWNIÚ}?ïÿø?¹ Â>ÔÚWNIÚ}?p+–CgJŸ?–)øvô©
?ïߨÓY•?–)øvô©
?‡#Ì7üp©?ÃAҖ?ï£pÎÛV?ÃAҖ?‰J,È*¾ª?z¼á:IªQ?ïš×L¶¶?z¼á:IªQ> @qÐà‡>Q¦ó<=Ê?ïÿÿþíA>Q¦ó<=ÊPSR4FGL J2215.6+5135?éN·¥-OÀ­6 ¥ýUÀ8̎eˆðÕÀ;þršQO~@kÛÎóB­@—‡B_ ?¦}	bvº?ÒÅ-¼PÓ­@#%">5ŵ@Wå¢0Áê¿·,£Þ'N_¿Ö§]CýÜ¿Ü-l…]¿ãý/5w±¿ìg ÉN=¿ëò¥Z'"PSRPSR3FGL J2215.6+5134PSR J2215+5135?xæžÚ÷?x‡‡Qý%–?ïÏô3B?x‡‡Qý%–?³Ê™{B"Æ?´æfŽ¦ã?톬Ð`³¨?´æfŽ¦ã?À<	L=?©¯†Eø[?ëðý¬ú°œ?©¯†Eø[?±ü(Ê*"Y?—i
˜zÙ½?íÀzæÈmå?—i
˜zÙ½?e+bÁ='?Xb¶Tψé?ïêÔ÷µûò?Xb¶Tψé?‹DÌZ-•\?"Ù9õU?ï'ìΗI«?"Ù9õU?"ô[¿­û?ŽY}1Êvˆ?ï`_DøÇ@?ŽY}1Êvˆ?ZT'íʾ–?KaÐ?ïòÕ·ø™?KaÐPSR4FGL J2229.0+6114?ïÉÊl}à@–Ü»WYƒÀ6þ"ÅõÀ:}E$Í>ã@ë
ò[ý'@h
"'r5?‰¥§Cü.9?ËçÂÇeYÌ@A[5Ÿôým?ÿ2̾_ Í¿¢T(÷(¿Øj¾[›¿âÓÄ"ïï¿åXåó€¿ì;E»Ëó‰¿îá['—PSRPSR3FGL J2229.0+6114PSR J2229+6114?gõ)º³?nòTK©È ?ïè<ø-ù?nòTK©È ?ž‹N v!'?¡'$¤ÝÂ?累

d?¡'$¤ÝÂ?½òÛ´T?©"Úy%b?ìA¤Ÿ©u|?©"Úy%b>)å^±ÁÖ>:ü¾›ø÷?ïÿÿþc®â>:ü¾›ø÷?]]V8ñ	)?Q¹H|?ïñQT‹<?Q¹H|?p¡ÝÕoò?xÔ¥Í?ïÞ¼DO¡d?xÔ¥Í?£"GÙµë? ñ`ÍA´"?îÆ»';râ? ñ`ÍA´"= )(U*¥Œ=VIâŠw÷
?ð=VIâ¹±9&PSR4FGL J2234.7+0943?ä§sMlÀD8ªà"À9WÿÚ@SÀ<*øÞ£@ 2×àÔ@-»à~í?²üPý+?Ú=ë]†˜á@!@åæyF=@
£Àäâ?ÛÛ°•^¡v?'9jYåúp¿ÚîädC '¿ãf0€ÑK¸¿ëùd€LP¿ïÿò^VÍlPSRPSR3FGL J2234.8+0945PSR J2234+0944?¬†Hº÷Ö?»ëžÛ3(2?î7›t‡ˆÂ?»ëžÛ3(2?Ò!p'ý1Þ?Åh—Ù{?æïG·g?Åh—Ù{?Æj\a¢(×?°
ix?êehç—uÊ?°
ix?×NmÁy‡€?µ‹…+cá?äXÉC<@?µ‹…+cá?¤°ɕ³ý?³¡¾¶ßz¤?î´øK'à?³¡¾¶ßz¤?¨´Ù% £y?°~™ON?ît²mê­ø?°~™ON?¼êG˜+A?³Ö B¬¤?ëPÅnõ0?³Ö B¬¤?šè¨/‹Y?‡Ào^}f?ï(º¾yÅ5?‡Ào^}fPSR4FGL J2238.5+5903?ï0.úqÿ?Þm:åÚÀ7tKAFò-À:×¥œàv@ßùߪu	@øB0üø? mXaÚªJ?Ó£{X)b@1¶®::Žq@=ØïÅË&¿ÈçV¦Tèæ¿ÕZºá'׉¿âø¾eUð¿ç‹Ýž¬(¿íÏ@ãȒ¿ïÿ÷œ"/¥PSRPSR3FGL J2238.4+5903PSR J2238+5903?T|ýŒ7?T£òó°ñå?ïõñÁ£ÎÒ?T£òó°ñå?£ä(l²e*?¢~WžÍ`?îÁ½yž^?¢~WžÍ`? kjˆê1Ó?—4NGRþ>?îùIWŒÙÃ?—4NGRþ>?wĝ-¶t?Î%­à•?ïÿTBȇ?Î%­à•?SÅ°v€?I"o÷/m±?ïötO k?I"o÷/m±?xjD*à?~˜|"úC@?ïÏ+ˤs?~˜|"úC@?ƒRü4Ë?fÙ¨7úÏ?ï²´f¥Q?fÙ¨7úÏ>o'±ó
™Ü>wv¸ýSE?ïÿÿà܊k>wv¸ýSEPSR4FGL J2240.6+5833?ïiBuÄ¿¹äÖg3À9eNÀWs"À;'ÊÇ9@¢	ç4'@Yr|õ%?¼*Ë/¾´†?ԞG=×&@³q*Ç?ó÷Œo?Ñ6þï´®?ë·3ÞSÝοÝá'ÑÖ÷É¿åÀʀAXæ¿ì䥜[d¿ïÿ¼ä!}(PSRPSR3FGL J2240.9+5831PSR J2240+5832?´Û·˜ª~?¶y攰7?ín‰ê°?¶y攰7?Ãñ+ô?±P£@?ë8¼Cµù?±P£@?Ö~E¢˜é?³æ{h è½?äÀÝ.³‹w?³æ{h è½?® C&ÒD	?Ž¥âe*ö%?îûͅP?Ž¥âe*ö%?'éÑ(rÙ?§4ːlT?ï´X»i3\?§4ːlT?•¾%é>_œ?§¤ž¬ê4?ïRШN"?§¤ž¬ê4?¢µeHã?•KàÒ]ó`?îÔ¯yw1²?•KàÒ]ó`?`HpékxÓ?Oð{~B?ï﷎Þ:ï?Oð{~BPSR4FGL J2241.7-5236¿ÑP‰ÀKw' ÿT	À8e½²}–.À;…ê&yçM@'´§«€@Ôœ¸2?¥W]bW?à¥Ç¥EŸG@6üa'?þr܎`ÖZ¿°±×þÚ,?£PAá̹,¿ØĤà¹)¿äƒÇ4ÝW_¿ïnàR»Ž·¿ïÿ»ËǔPSRPSR3FGL J2241.6-5237PSR J2241-5236?JŸèΠ?FéŒwhÎÛ?ïùX»fb?FéŒwhÎÛ?Æ%G5&[?­¦ »Œ^?êv®2¶i<?­¦ »Œ^?•&–QAb?q.èâd?ïVËMh5?q.èâd>éK;–}Ý >ð™Ë-pþð?ïÿæ´ÌÈ=>ð™Ë-pþð?Pë$µx?CZÑ?j÷¯?ï÷Š?€ëÅ?CZÑ?j÷¯?«÷	õÞ?«½Ti Æ?îO7s'?«½Ti Æ?ˆHpãì?}"äø²ï¯?Þ5?}"äø²ï¯>1¨Ê_M>\Žõ5VÈ?ïÿÿýÚ>ƒ>\Žõ5VÈPSR4FGL J2256.8-1024¿ìlÉlù†ÀM#b¶®}VÀ9¥[n¼À<EÉGÝ@Ž%·õz@?ÿbîᵒ?µ¿'Ò€?ÔGÁSœà@éö©?)@k • ãû¿ÒEI€|'"¿Ó¶z¢Þg¿à*‰
ÖØ¿åEcKÿ²Ó¿ïÿ/àîAè¿ëw´!ZBÂPSRPSR3FGL J2256.7-1022PSR J2256-1024?ÚáʊÓ-?Ò²Å"ºÝ?âøº–i?Ò²Å"ºÝ?åû5è+a?έòN?Ô	"/ï©=?έòN?×þ	f—J?µgjɔ·q?äðûL´[?µgjɔ·q?é?ß$Nz?«/˜ÇR2©?Ë·ƒnÆ?«/˜ÇR2©?¾¹ÛaЊ?¸Le|d27?ì(ēÝï?¸Le|d27?ÅM›¯|?ÉdÀ‰r…?꬙=Ô ÿ?ÉdÀ‰r…?Ç2˜\òc#?±"Ñ
1!Ú?ê3YèÃg7?±"Ñ
1!Ú?Ëë±`×þ|?·ó9ýX?é§Êa?·ó9ýXMIXED4FGL J2302.7+4443¿îÌÅNkTÀ+ü"«%³À7ý#!m8À;ŸDÔE@§ó3üÝ?úæé¸?Ÿ7‰.<~a?ڔšCã…@9AÅ3?öŠ¸³:T?ÒCÛí㿦ašNË?.¿Ó$"ô÷ŽA¿áÓ{½™Á¿íFñVI¿ïÿ°"—©ÕPSRPSR3FGL J2302.7+4443PSR J2302+4442?j1÷H?o0»Éï?ïåÎ	?o0»Éï?£äV3ë ?§f*‰€?îÁºœÀâÖ?§f*‰€?'ö¢üGMl?‹+ã×­î?ïpJçôŠE?‹+ã×­î>¢:âV.×>­®C¬?ïÿþÜz¥õ>­®C¬?ˆ…ü˜gL?¶?=O
PÃ?çÖ¤£?¶?=O
PÃ?2ÿ5D¥_?Š:ÙÆå•?ï»4<Ëb?Š:ÙÆå•?"}1´!?n›aÓF?ï®9!½H?n›aÓF=Ýûµ­"MÑ=ùŽ‡žÜ´>?ð=ùŽ‡žÜ´>PSR4FGL J2310.0-0555?êËß@åíÀLó5*"8	À9ñº
RiYÀ<ƒ6ª¶øO@bsN×(›?û_틉5ž?¾rø-}½?ãáKŒ]@!#{ñèæ@›ûcŽß?ïöý»'"?ÒýŽ`«fv¿ÓfF…öN¦¿ç<ù jn3¿í×ÆZÂÄ5¿ïÿøÞ£ŽæPSRPSR3FGL J2310.1-0557PSR J2310-0555?´*¥Ãdy?¿aoq'	¯?íz«GÊw'?¿aoq'	¯?ÎÕ^iW?Æáøý¥?èJ¾¨zeª?Æáøý¥?Ëë ]~Ç?³ïG,™£ñ?é8·è N?³ïG,™£ñ?Ư2Š8J?®?†J(åt?êT3]qí{?®?†J(åt?†)D©H?¨œ­`¥ü?ï§Zï[?¨œ­`¥ü?¨×†Ì"Ýï?¯Ô»E™p?îr‡"K'?¯Ô»E™p?«Ô•‰´"?¡{¡ó?îB¶§'¡—?¡{¡ó?ŽNf˜Ïêð?'äÙá˜ÃÔ?ï†Æeª~Ä?'äÙá˜ÃÔPSR4FGL J2317.3+1433¿ï½È'Ã{ÀE;^Ès¬À;•'àÙìÀ=$)Ùî@¾CdÞØ@'#[NÛ/?؈•zѐ?ïÿ–ل@£ÃÙß@4ÛÐË´õ¿ïÑ	ro‰%?ïüٍ©Ì¿ÔóÉ[(Dÿì¾YÂi¢¿Ð×ͱÏ…¿ïÿM½øôsPSRPSRPSR J2317+1439?ëNg¼§»›?ÂԽؤWŸ?ÂÆa
a"?ÂԽؤWŸ?ìë¼³hçd?ÀhÂä8Æ?¸¢e"«ß?ÀhÂä8Æ?꫗+'d}?«á‰‡Óžx?ÅQ£Qºn?«á‰‡Óžx?ì‡ë·§)X?¥'g¾L£¿?»À¢BƵB?¥'g¾L£¿?çüã½µ?È7ö
!°Ä?Ð8…Ïږ?È7ö
!°Ä?ÜÒdÍpG?Ô¨ÍÄn"m?áò͙GÝ?Ô¨ÍÄn"m?äM¿ŽÔLQ?¹òLEÐ?×d€âWg_?¹òLEÐ?ÙÆçýÍB?Ýõ^fg¾?ãŒt_?Ýõ^fg¾MIXED4FGL J2339.6-0533?î<âmŒº'ÀO<Øý\·'À8Bj4Q@À;Ítj5(@à,Ä.B´?úê°¢¥²?£ÓցVÂ?ҝ)[™ñ@0í·'êy@é\‹{õ?ëVáŽ$ñ¿ÒÅ}Î¿Ö.ºJi¿á^n€[˜¿ìÂåÃ=Ø¿íˆdüPSRPSR3FGL J2339.6-0533PSR J2339-0533?Cšs.,?'1(»äx?ï}ã,'€?'1(»äx?ÂY²fU?Á	Ò¼¥ã)?ëi"yfj»?Á	Ò¼¥ã)?­ß£ÛBÛ?¢<8ƒhЅ?î"Åë‡"?¢<8ƒhЅ?NžÖüTw'?Ky`⎻G?ïøXIÿ8Á?Ky`⎻G?pÿVÎuÞ?ræ6J'?ïÞRp¦?ræ6J'? º•ñ!?¡¤Ã‡=q\?îö.ô›Y?¡¤Ã‡=q\? /-Ǽ×1?œ
žӋ?îý
#vt?œ
žӋ>ËÌà'¾U>Ó›]ôîÃ?ïÿùÏNæ>Ó›]ôîÃPSR4FGL J0002.1+6721c?؎*±b@Â[T‹À9Ð'Ai
À;2ɪ@o£c@ëˆÊ>}?Ê©>þž?ÖmŽcZ˜R@¦÷ µí@S³Ü:ÿ?Ø3ºâ¿}Y¿æ­ݨ<J¿âžâ^.‰€¿éB"ßοïÿþ½à ¿?é§fN³OTHERunk1RXS J000209.4+672503?å}ÛÜùÚf?Ç¢sxÙÁ¹?ÕHFK4?Ç¢sxÙÁ¹?åA«_1?Î^ð^?Õ|©ÑAü?Î^ð^?è×Vfûý?­\It˜Ò?Ì¢¦dŒ
?­\It˜Ò?êaò6Fk¨?©ï=òÌ2@?Æx7&æQa?©ï=òÌ2@?քnênsP?ÉõÛpËçl?ä½ÈŠÈÆX?ÉõÛpËçl?²ƒëÍè'?¾Dˆ‹Ë?í¯'†yùŽ?¾Dˆ‹Ë?Êm¯
§»ú?²ã" ¡Ä¸?éd"<–?²ã" ¡Ä¸?¿WR³g\A?­r‰B0›?ì©"x?­r‰B0›)MIXED4FGL J0002.7+7220?ï‡sRnH@#¨–»˜ÇãÀ:hã1" À;}¹?QN§@e	Àóû@H_ÐJ/Ï?Ð<ÌÄ¿78?²[¿ïCÅ'?çFùž¼ï	@HF6p)‰?î–ÿöÅě¿ÖOæ<Štä¿å	Ñ:×B¿ä"è™¿ï'Æ0ÑY$?âãA&
OTHERsppSNR G119.5+10.2?ïùÈΐqR?oØäf&9¢?HÜÅÜwH?oØäf&9¢?ïìo®òñ?dáŽìê"û?cQ¤"ïË?dáŽìê"û?ïŒ[µˊ?ˆ<ÛY€Åz?Œé£|¹'?ˆ<ÛY€Åz?ïÝ&!ZvL?XêÏЍû™?qlïV4v?XêÏЍû™?ïðéÑâ­¬?_LÑ#Ë×?^,[ÏpØf?_LÑ#Ë×?ï"=
'BL?"Æ[ƒ.TC?Žð½X?Ñ	?"Æ[ƒ.TC?î ¡B°SÅ?Î+e—0?¥õëÒg¯?Î+e—0?îáú—
&?':0A=ê?¡àV'c•?':0A=êAGN4FGL J0024.0-7204¿Ù€°á×ÀFr¾ß¤@À8Yø©ÊiÀ;òkón!F@y§¯†ì?ûäû,[¨?£g¿j?Öìþ{E›–@4¸Œ£è?ú"Ï»¼Ë?ހeëí#"¿¯kR3~‡š¿Úàr%uZ¿ä.b"óè¿íè«ð´2¢¿ë©;}"OTHERglc3FGL J0023.9-7203NGC 104?týÃ!ÃÃ?s‰¢'#÷?ï×ØI¡ñ?s‰¢'#÷?Äa
+a­š?¿É8qû3×?êç¼µ'"™?¿É8qû3×?žj¼Èƒù?"'›Â—(v?ïª»à8?"'›Â—(v?Æ[<¨x?`"[\èð?ïÿYÌúïö?`"[\èð?e¥÷	Z?Y–X7Îw?ïêpZAP>?Y–X7Îw?§9Ó"‹Ìü?¦‰si€¸|?îŒbÍ»ÆP?¦‰si€¸|?‹5>¢¾`—?€—==2Œ?ï"+gH?€—==2Œ>t<&{Ÿ>}ì|›)?ïÿÿ×¼>}ì|›)PSR4FGL J0025.3+6408?è4ˆ;"k?ö¿ã°> ÍÀ9Yº !ÞwÀ;'µ‹g§¯@ "CÆS`û@dŠ=Ü¡?³á_èE?ˆ´¼¾?sç?ÖH¿aÕ2?÷>ó/âò?ïÿjCj¸Û¿Ê˜†t"è¿Ü•qaEg¿åÏ2ؚ`i¿á"?Žò¿çàÌÞë]\OTHERsnr3FGL J0025.7+6404Tycho?ï»KÄéBh?¨i	p ŒX?-¼~?¨i	p ŒX?ïŒ\Ú¡v³?•b`ål-?ŒèÉañ'C?•b`ål-?ïnÂ!fñÀ?ŒÍ¦Šš'‹?''»Ö'cî?ŒÍ¦Šš'‹?í½|ÝÌ#…?š¾ÊØ5H¨?²žãÛ?š¾ÊØ5H¨?ï®"‰©%?{ÇsQ?"xäÌä›?{ÇsQ?í	05°n¦?½:ñK9íÀ?·¶~SÆeO?½:ñK9íÀ?ï
]heð?–®™.Zsx?ž\VbÝý?–®™.Zsx?çMFëÝðG?¶,¬våp?Ñer(Dr?¶,¬våpAGN4FGL J0043.2+4114¿ÔõeêÕÌÀ5š¬§"W`À;
"ßþعÀ<fI¿f²½@-¤€¨[ÿ@0\"U?Õ'،°?æPràÈ,@M7 '½´?öؖVîú¿ÞDD}ˆkõ¿¬¸€‡qú¿×Ç
â@Ò¿îž/á5¿ïÿ¼þùoÃ?≲€ñ,(OTHERgal3FGL J0042.5+4117M 31?îØTè8?¯§í–Dà?¢z¿?ı¸?¯§í–Dà?æ<ZÄû$Ø?ËþÃêÐîÅ?ӇJv	¶Q?ËþÃêÐîÅ?é›Ô=ÚV?®›SRïX?ɓ¸¯–§?®›SRïX?èj¼r½?°ÅôÓ_?ÏîU5‰
?°ÅôÓ_?ì¿w'fR"?¿ü;ÍO?ºClÍnï?¿ü;ÍO?À8¹QgH?Ân"|è3?ëû1Ñ«¦.?Ân"|è3?Öï¾vc?¼.ÁÒ{k?äˆ öDÀN?¼.ÁÒ{k?ÂLv…îA?°Bûâ'ì?ëlâ^"o¼?°Bûâ'ìMIXED4FGL J0047.3+6943¿ïõûÃ
@iìb"IÏÀ:ç¬è*÷%À<TBcQÞð@!BcMØ%?ÿ*'5Îîæ?Ê=£N¤(?¤0bp-?Þь"Þ ²?üë¯Ï;¿ïÿª¥Z—ü?ïø;`(^Ä¿åÑ3~²†¿Û"½'Æf¿Øþìɹ¿ãMòfºI=OTHERunk1RXS J004724.5+694222?ïþ<«?$ªö$Uæ?,7噀?$ªö$Uæ?ïàJÜ®Rt?{ŸÕ[†Jr?oµ#"‡Ã<?{ŸÕ[†Jr?ïëÁ1c$h?nØæ;(å?d>Ξ;pk?nØæ;(å?ïÝÒò3lG?X…$µ?q†Ö{¨¿?X…$µ?ïþEå+W6?$"²GpJÖ?+¡®@×e?$"²GpJÖ?ï(…Ú—]!?¤/1þ¢)X?šïD®Ì)æ?¤/1þ¢)X?ïê–òJ_Ë?s‰¦…Š?ei
~¦u¶?s‰¦…Š?ï(´¾–²?òÙëˆ?šÿÉh-)É?òÙëˆAGN4FGL J0047.5-2517¿ït.VÁ•ÀUþ	þ†ƒ<À9¸×ï?¾\À<'~b¯@¿jë@,^,Ü?²zãáfaß?».Ï¡=|ã@	þÂé<@RÙâ)U?í8ÙÀ¦"ê¿Í]ª?¯…¿áÁVw¿ãú¯É†Ç/¿æ´EL:k6¿áágßjrOTHERsbg3FGL J0047.5-2516NGC 253?ïöÉщ?R.‰áÛɵ?Sèl>°R?R.‰áÛɵ?ïÌ@_Q?"PòÙ_"?yýßænWK?"PòÙ_"?ïÌ¡3Êer?|ù'»£?y¯fŒöþ?|ù'»£?ѧ…ž?nÔã¾ù?‡˖˜z?nÔã¾ù?ïူên?nüu÷@ë?nNÚxšè?nüu÷@ë?îÆÊ.·Îc?±ÑÃyä]è?£"]§2Ò?±ÑÃyä]è?ï…¸»-?—9%‹`ãô?Ÿ/Hÿšj?—9%‹`ãô?îEã.cÍ?•†ÜHWí?«¡Íγ,?•†ÜHWíAGN4FGL J0058.0-7245e?éNÐà$9èÀF/Ne¾ ºÀ8f֕£jÔÀ;~ÚÉÒ+@<›=އà@üÅ2¤—ú?¥ª	ÜÖ7ã?·e~"é×@ò–pm@Pބ°(|?ïZ˜1º/¿Ü°žBö ¿ã1Í7U×£¿ãdâ¢÷ç-¿æí¾Ña‡¿ïÿDN
ª
OTHERGAL3FGL J0059.0-7242eSMC?ïm'påÎÚ?–hœ÷?'[ãF$Á?–hœ÷?ì/:zÐ*Ð?À×°ÐÖ?¾†,)~©~?À×°ÐÖ?íRœÉ5#ß?¢Ëóö*–?µkµèí…?¢Ëóö*–?ë"òh<ÕH?£\	Ëϯ?Áì6_ªÞ?£\	Ëϯ?ëjWo±t?¾Ó;Íqɂ?ÂV¢A;'0?¾Ó;Íqɂ?ÜkÝ¡äÊM?Ò¬­iýl?áÊ/
šÙ?Ò¬­iýl?ìKÄúpt?¨ù¨éfã?½¡Ø,|_Í?¨ù¨éfã?׌CªÏ¡é?¹?Î?ä9Þ*˜/?¹?ÎMIXED4FGL J0059.7-7210?ìäHRîÔ"ÀFwè¢ìÀ;$¡¯ À<pƒåÓ.@;uÒêóÿ@¯0¿»lR?Õ~aDh¶?ëc݊Š2@4	t@¼•Dj¿îÍ=ø:?åüO{пç£ôÑΔM¿íç	Ÿ&¿ïüÖë3À!?ã'‰|$TOTHERsfrNGC 346?ï7ÉA@ÖÏ?¦'ar(?™×ÛTÂ(?¦'ar(?îÖ¸©õ?¬p˜¯¾èì?¢"{Ñ«°?¬p˜¯¾èì?í-ŽûÓB?£ï"*§?·þ"†×‹r?£ï"*§?²²*›?'ãë;;¯?§×TÙ(ÙF?'ãë;;¯?ìÛ1§AøÉ?»æ.ȕZ›?¹&rÇ:8?»æ.ȕZ›?ãý'°ìò\?Òɧ­ó?Øܞ&H?Òɧ­ó?áUêj#?¾"'êw$?ÝT++ãïº?¾"'êw$?à¨M]ù'?ÀïXõ±êÁ?ßÖ¯eD
²?ÀïXõ±êÁAGN4FGL J0102.9-7051?ïýb¸ ´°ÀG¡ô±îÀ;@X|™À<Ȟƒ
f@ñà¬Óˆ(?ú¹_ÒÎn?ÙjCä'?éäNÿA"@uPÊï$@š6ù¼D?îð0Ä#¿íÝ.yÖ?Õç[ƒßH%¿æÐt!:k¿êÿsFT¿ï5?†'ÍOTHERglcNGC 362?ïúø*ð·?C8¹ÏL*µ?DW6øœó?C8¹ÏL*µ?ïó S5÷?ZÇíAì–?XĿLJ'Ð?ZÇíAì–?ïoâìÒY\?…¦³ºUq?'¢e´Ôw?…¦³ºUq?ï¾D]@ç–?n2vÚLÉ?€nè®L?n2vÚLÉ?ïætÈÌ.?mE<ýŽÅ?i‹7õùŒ?mE<ýŽÅ?ïÖw]¯ˆ™?}4á)¢§?tÄQ­Ïy?}4á)¢§?îé-ö6?—EΤÿ?¡m/ÒWZ˜?—EΤÿ?ïM4Þ{m?ƒíë­Ò?Œ¬²º¢´¾?ƒíë­ÒAGN4FGL J0138.6+6821¿©Ënš2µ@ƒÅ¢6 MÀ9Á%q©ˆÀ;‡tߥíe@7fÛ¬8®@ú}ªOÊC?¿æùß)›°?³u67õdÆ?ó®K½m´9?íý°ðMZ?ïý'w>$ÿ¿ãþyC¿ë-Z˜¿çM	h^Ž+¿ä©,I4&x¿å¹^Æ^ô'OTHERunk87GB 013451.9+680621?ïâMMÌ͵? Ö·Í°NF?m²±ý˜c? Ö·Í°NF?ëI•µ*ç?¾ é͗*²?ÂÙ©+Tcý?¾ é͗*²?ï
³Wô†?'Ê0À[2'?žI•"Ñ,?'Ê0À[2'?êïgl~a
?¤44]QU7?ÄBbN{Î?¤44]QU7?ï%÷#əù?¢cbÍk?›A‹ô*å?¢cbÍk?́O;ü[?ÏAÜ0‡û?蟬:±é?ÏAÜ0‡û?íœ(ðd+¤?¢ÿA'g8?³¸{&Ôå?¢ÿA'g8?ͅÕí\å3?²EûmyI%?螊"¨Æ³?²EûmyI%MIXED4FGL J0212.1+5321¿ï"ØÐnËmÀ…‰ïØjÀ8ÚÓC"LÀ<|ûÔ!U@Å0L£òŽ?ýàBæ.¢?«ØB÷¡aº?ؚÐÑ>K•@)0"»?ö­—}_§¿ÙÎ"Ë+b¿µèüoq¿Ü¨b_EµÂ¿åj	=ìIÀ¿îeÖS^Kæ¿ïõŠ@`B`OTHERbin3FGL J0212.1+53201SXPS J021210.6+532136?cƬLþ¤?añAr"s©?ïì9S€'$?añAr"s©?³æª+}«?³s#íë·f?í*¬ÑÛ?³s#íë·f?›"tüþ¯?'ûƽ+Ö?ï'C܁SZ?'ûƽ+Ö?bG
<nY?Xeؽ?ïí¸õKéZ?Xeؽ?`jù‹+H¬?P´‡:H0?ïï•6ûÀ?P´‡:H0?Ð
jç¸?•É÷Þ²ù?×à•ñ?•É÷Þ²ù?…Äe&ÁŸ?oKów÷'}?ï¨îkƒÙ?oKów÷'}>ï%7!VoÄ>î¸î0&¬2?ïÿàÚî>î¸î0&¬2PSR4FGL J0221.4+6241e?ÜòDŒ],<?ù—?·¥ôÀ8PÃí*:fÀ:ˆ ¼8*@ò§|Ü@@dß}©y?¹S;€""í?×|CG}m@d@y?ô†@Æï" ¿ã¸Û~@w¿¿¹Ó/<ƒ"ô¿áÃGb• Ž¿é@>aÔ¿í)Ãèø|~¿é+
oÆOTHERSNR3FGL J0224.0+6235HB 3?—Ж:©?¦Y_æÇ)?ïASi«ã?¦Y_æÇ)?¿® ÂËÊ¢?¼—¢«]ˆ¿?ì
;禆¬?¼—¢«]ˆ¿?ÄÝô§¸?°`<OÃ`?êȂþÖù?°`<OÃ`?¥©Í.è;?‡Ä.®ï5:?î¥c.xŽ\?‡Ä.®ï5:?iž÷á%Z?e'™zùW?ïæì`ïa«?e'™zùW?'Ä?×Ó³h?ž'É~‹6°?ïiÞAbe?ž'É~‹6°?X˜uì¼?}F£LÓ?«æ½?}F£LÓ?F§cš·i?6ôó1³ ?ïúV' w¼?6ôó1³ PSR4FGL J0222.4+6156e?¹Bä9d u?íõ,ÒÆáÑÀ6ã'[·¶»À:;`z"@½…TÖ@v¥xÊí?š±Œ¼ú?л0J@0}?À	oë@âFHä S?À›ïà"?¿Ó5"FK=ì¿ä°>Œ,ɍ¿è*¹¢"ª$¿ì틉5žG¿è=¦S¼?·OTHERsnr3FGL J0223.6+6204W 3?"ò䲞W¬?¤F®0Ç¡~?ïXhÚ4ƒ?¤F®0Ç¡~?¨Ò×»®»l?§õí]V–?îr҄`')?§õí]V–?¾–+|s?ª¹]'Ùì-?ì-:ðn?ª¹]'Ùì-? Œå½®cG?}ñ1þ|?ïþ÷1ØÈ·?}ñ1þ|?jÖný/áZ?–üùmó+9?ïå)'/÷?–üùmó+9?~¡±mÜ4?"ý®×ša?ïÃÖ¼dÊ°?"ý®×ša?˜8³/0´?'#í$nõ?ï>?Z!ÎK?'#í$nõ>{"Áv˜L>ŠHÍå$Û?ïÿÿȳɭ>ŠHÍå$ÛPSR4FGL J0240.5+6113¿ê$â§Cj?ñfþÂ^§À5zÚÿ•wÀ:èâ­â@P'ԅRæ@0Ҁjôk?~>n-bÂK?ÂôæÇIÖ
@=[oâæê…@Vo"w¤¿ÀNÿYfú¿Þ‹É'—½¿äæMà^¿æŸŒAœƒ¿ë¨{Ÿ2µµ¿è,¿0|uOTHERHMB3FGL J0240.5+6113LSI +61 303?îdìáÀ?·ƒ¸áÒP?¦)±07uû?·ƒ¸áÒP?£~$lG±,?§mKËÅ
Ã?îȹWÍ?§mKËÅ
Ã?å輨Ž?µ4ó™¹Q?Ô.†¯ËÎå?µ4ó™¹Q>ñ
ÑC©w>øʘtq?ïÿÝåñ-w>øʘtq?è'ÈÄb?ÄlÔ+]HR?͸Üïžw¿?ÄlÔ+]HR?uŠì͇(œ?~Q‰)ÔÛ?ïÔê&"¬_?~Q‰)ÔÛ?çyŒÚ?·|¹Ï 
?Ñ
ÞçùÆL?·|¹Ï 
>®úOÿœ>QùrË
íÃ?ïÿÿþíA>QùrË
íÃMIXED4FGL J0242.6-0000¿è™ºî†ÀI÷%€ÃÿÀ9ÁN_¤À<Iʳ!@æG¤€@'šCㄟ?±ï¥ö,? : ×ùÒ?ë~‰¬¼Œ@Iύ¿âuác\ƪ¿ÝT»ÊàŽ¿çPÝ»1š¿æ?2Ȫ(¿ÒKÃãD2Š¿ïÿŝƒ‰OTHERsbg3FGL J0242.7-0001NGC 1068?ïþ–²'? 'ꘟ$œ?.f•,¡¢E? 'ꘟ$œ?ïö$Ö4eÉ?U¤¯ï;͏?S¶SÛìœÃ?U¤¯ï;͏?ïðH˜j?[.?Jo?_næLƒ›ë?[.?Jo?ïüoÝ]"¯?(¸.•&"?<¿Lu?(¸.•&"?ïüœ¥´ýE?3St—dµ?;Ñ:6\?3St—dµ?ïÖ$32?{$ÑÜÜ-v?tðmþş/?{$ÑÜÜ-v?ïÖ»$Ñ#?|§	l®à™?t¢m§õL?|§	l®à™?ïðéè*²?RA§QB?^-Õþ0;l?RA§QBAGN4FGL J0328.6+5330?êÞįÙTÀ­È"#^À9øxG9zuÀ;£ãŸw)@ùqcÅwC@öVhÂa9?ÈBÎFIm?Öiü¾, @€_&×@
$àŠó?ï­Ä~Ÿ˜6¿¦=žàÅ¿åkB£é~´¿æ–akTâ°¿ïý®KØE§¿íþyzϪOTHERunkNVSS J032847+532859?íTiŽ¹í?µ<{p³?³•\±do?µ<{p³?ä¹ûÃý'µ?ÉaAsì?֌xږ?ÉaAsì?ìH6é(֗?£¤LNX—?½¾H¶¹KL?£¤LNX—?æ

ˆ¢®õ?¥ªw}ß?Óëê?¥ªw}ß?ãg}I¿ä?ÅèõÜTn?Ù1mʀ9?ÅèõÜTn?ÀˆâÅ»E?Å¿°|£á?ëÝÇN';/?Å¿°|£á?Û|QZX?¹Ò\ ðÄ?âAø×RóÔ?¹Ò\ ðÄ?½
c'†?#IÝÎåœ?ì^SÏ> ?#IÝÎåœ	MIXED4FGL J0359.7+4445¿ëkÚé'w´À0=µm5À:P "ˆÞ`À;æÝî]@M@H¯å`l|@È!å-ã?»ú# Ä¿©Œסçò?ïùÓ`dĦ?þ"EÇ	"¿êf"¿˜?¿'X¡p—\¿ìÏÀÒÆӿטh û£$¿ë^>¿ƒc!?áÏÐÝӅNOTHERunk1RXS J040006.3+444512?ïí'~8ÙÕ?cWR?œ†â?b}'ߚ£?cWR?œ†â?ïæ:«ç;?pd ‡P> ?iÅTÅ>Œý?pd ‡P> ?ïTñ¢«L[?Ž6ÇHéî?•a˪–tª?Ž6ÇHéî?ïÜÔXv'"?XŠm°sW?q•ÓÀÂY?XŠm°sW?îôՋÑô™? @¼ Ã~? ²§C¼t? @¼ Ã~?ïê[¸;?­GÓ63É?´‰`Ƨ?­GÓ63É?î¢Ü¢¨6?šûkñ•®þ?¥Ò>&±cž?šûkñ•®þ?îOm˜J?œg~¯×u?«Ù,n­d?œg~¯×uAGN4FGL J0402.5+5402¿ßfš6U/:?ðƒ
%ó¯À:ÔüøÀ;ñ4ØNá@"7ÑÌ?ÿx¹º¡Q?ÊÜ@Þ¡,?‹`Ŭ`àY?¾Ó¯êéÃ@›ØÚ¢"?ÔµŒßvó|?î<xVRó?›PÇåÿ›#¿æ—œ~ÑAQ¿Û0cu^P¿Õ×Ýašy¾OTHERunkTXS 0358+539?ïùòAY?xÆÕ`ý?K€7Ó6,µ?xÆÕ`ý?ïæÉܓ¥u?vÞÛõ4!?i6#s9Âö?vÞÛõ4!?ïåòºb+?qšÛëÓ+?j
ôe:<ø?qšÛëÓ+?ïìэYwô?OãL@eÞ3?c.r}L¼.?OãL@eÞ3?ïýgN:B?2z°þé?4ōÐzÎ?2z°þé?ï1ãАå?§Â7œŸ>'?™Ã…ó–Ýt?§Â7œŸ>'?ïÍÜéòÄÐ?R¥×þù­?y‹K¥?R¥×þù­?ï¿iKY›?sL®É0}?€%¿ŸÃi?sL®É0}AGN4FGL J0427.2+5533e?ë5ºOFº@P;£D=GÀ7éè¢ì(³À:Ìûƒ¶@"JjꯋÉ?ùV~AN~é?§þÅdÆ?´Æ´"×j¶@Á`@Q{Œ=e'¿ïÿòɶ—×?ïþÀ//˜t?ÔHk^rÒ¿Æ­ò2ql¿Ôàœbvª¿Õ¥µLOTHERSNR3FGL J0425.8+5600SNR G150.3+04.5?îþëWó(?´¿™–Z? N¸Èÿ{?´¿™–Z?ë`U'h.?Ç^áÈî'?Ãî~©º_H?Ç^áÈî'?ë =áªL?­çp郣?ÐyVÐ?­çp郣?é6"‡gÔ?²)¶¶þ?Ë%íã¦`°?²)¶¶þ?ïJÞSÄ"?—ÉkoŠ©?–¤5Œ¦Wr?—ÉkoŠ©?âöÝÂhoÖ?Ôó?}Cx?ÚD{/ T?Ôó?}Cx?첯û/áš?«eÖ&El¤?ºj€&€ó0?«eÖ&El¤?Ûp‡5­¥¯?ÂvÞN«_?âG¼e)-)?ÂvÞN«_MIXED4FGL J0427.8-6704¿ìµ¹×ýÑÀCFž<–‰DÀ9{"ÆäÀ<XÚ")@·«N!÷@þxük 
?¬e BÖr?"~­Úï$f?äsÂÚۃI@ïÒ#ù¯Y¿äÂB…5´¿Þ
÷9‡á¿æêL¼ƒ©¿äy'EÖ¤¿ãà>>T#™¿ê˜iñŽOTHERLMB3FGL J0427.9-67041SXPS J042749.2-670434?ïüÁN¿UÁ?.Á5oƇô?9õ‰qüSØ?.Á5oƇô?ïõÜhKBô?VγÈ=Ë?TG/»ð¶«?VγÈ=Ë?ïæµÂ«Fü?p»EÁ£I?iJ=€´t?p»EÁ£I?ïðay[z?O¹|¯!Ê?_Ç=ˆ#?O¹|¯!Ê?ïùHßÙ?CHoY	a?KæÞ?X!o?CHoY	a?ïØCÁ~m¢?|¾xù€N?sÞHXS?|¾xù€N?ï¼¹ƒ2¾³?"f^°nÛ?€ÑŸ5¸
@?"f^°nÛ?ï»éòAY?vE±—ì‹?¸/Y¶?vE±—ì‹AGN4FGL J0452.9+5117?Ý»•0Ã=@…‹W"<À9Ò¨Žÿâ¤À;m0•Ê@@ŹE˜›@¸PXÝç§?ÇZSÑä?Ö¥¯Q'Ã@é.Àë­@ݜ²üÂ?ÎK™›òå:¿ÔUäswÇ¿ç-v% Jù¿ëð\>D^T¿ìí8™¤¿ïßøÞ£ŽæOTHERsppSNR G156.2+05.7?ï_ü¹hZÌ?·"q*+ûñ?"hÍÍ<"?·"q*+ûñ?ï
Ì$mÓ?¡lrd¹wŒ?ž¦{{â©¢?¡lrd¹wŒ?î?´^K?™»ýÚ|[ó?¬¿
W?™»ýÚ|[ó?q³v?€©Ç´"¹?¦XáXû
?€©Ç´"¹?ìôKjaž?³;ä•gò?¸_¤¬ó?³;ä•gò?æaz¹"›†?͟ô­ø‡w?Ó=
ŒöÈõ?͟ô­ø‡w?çÁµÂo&?³ð2^uKõ?ÑÒ|"{!´?³ð2^uKõ?ã«ò›8f?°è,ÂFZ.?بÐɏ3?°è,ÂFZ.AGN4FGL J0500.3+4639e¿ï¦,Zãº@‡?i¢[À8:œÄÞÂÀ:ÊØ£š¤@ïCÿ‰8@:–¹ëH¹?±®+L	?Å2évј@k˽Ù@ÒFö^—¿£—ìÆ<e¿Ôä±z¶Õj¿æ×2ƒ2¥¿ä€µ¿ë%F Û¿éøDŸÂ'­OTHERSNR2FGL J0503.2+4643HB 9?èâ+j€Á?Ëa‹Ñž²?ÌwRUüûƒ?Ëa‹Ñž²?ÜkÃʒl?Ëï\!qZ?áʶÿJ?Ëï\!qZ?çU«ëçÖ?²ò¡Z0·©?ÑUè¨(0S?²ò¡Z0·©?æÁFÀ??¡ò?\à?Ò}róé?¡ò?\à?Á¼'Aïí?Ã$b_?ëß|/"?Ã$b_?§ 8¢<?³mZx"Üä?î…ÿÿ‡½­?³mZx"Üä?Ömä°ªh…?¼yg!o?äÉ
§ªË½?¼yg!o?½JcY\ë?üüA¥)?ìV³"Ü4c?üüA¥)MIXED4FGL J0517.9+5030¿Õ*Kƒ8@NÏ~Wô´À;í$[)À<uŽÀøƒ4@×̃%äÁ?úÒ
#opÑ?ærÙ;p—?ç©8¨½ùË@;šÅ都?þGÙbÝDê¿ïüD=é?ïþašNË?¿ãÇ}Øró¿Ñ}Nñݨ¿ìÄÝëAú¿º_Êø®OTHERsppSNR G159.6+07.3?ïӔJ¶mÌ?sÓô:¥D?v5ڒë" ?sÓô:¥D?îѶÁr¦'?¨ÃV´8
?¢ä"çÈø?¨ÃV´8
?îE	NTÄ?™°Wv3÷?«¯k#Z?™°Wv3÷?íô=ÊÄg?'Áô2•Ÿ&?°^¨$õù?'Áô2•Ÿ&?ïFÜ]cˆ? šfû–ø?—$k¼ˆÿ? šfû–ø?ç­6F¸÷?Îw=Ñ>Bþ?Ð¥"rŽü?Îw=Ñ>Bþ?ívôýÝ)Ö?¢ùÞ¡ã†?´HXÌÖÒ?¢ùÞ¡ã†?晵}r>?¶Ò> ='u?Ò̕ƒû?¶Ò> ='uAGN4FGL J0519.9-6845e¿ïñ¶°À@±'¡ ÏÀ6îñ<îØÀ:\pšœÎØ@C¡lv˹@Z5þ¿Ž ?˜Óy—ϼ?ż°µj¬@,H2ËŸ@5ëq…¿À²ŒÙÔG¿ÒÄË¡~•\¿âóó¢y'¿äªúêíID¿êWºÁÝZ¿ÎH"•sOTHERGAL3FGL J0526.6-6825eLMC?°/`èš?¿¦/û¬op?íðýbí?¿¦/û¬op?Å.(>Yú??À]I
¤¸u?ê´uðip?À]I
¤¸u?Ú5›Wã?´³xºgJ?âå2|Tu?´³xºgJ?uFü}¼[Í?o©^&?ïÕrúè`?o©^&?£'.˜"?Œ'ý0S?ï¹q÷ÐAÞ?Œ'ý0S?¨wÞ-Ô@ã?§#0Çù?îx'Yµ²?§#0Çù?Ég+Æ°?¸½€—~²?é¦8µ{T?¸½€—~²>í'eOçC&>ñ˜"ò$eu?ïÿâ}°|W>ñ˜"ò$euPSR4FGL J0521.2+1637?Þ¥©ª*WåÀ&©O‡À:–E"I$À<!]×MY@ëÉa2tò?ø~Ûrýœ?؃b¯É?ïNH,¿{«?ÿú"5¬Š7@ŒÕ»Þ¾?êfÆ"Ž A¿èðaՈ¿Õ@˜Á­^ó¿àåQÉ oâ¿é*‹"ÞQ¿â9¾'‡.]OTHERcss3C 138?ïõÕÎ9oŸ?`fCÛ½z?TTc5*Ãq?`fCÛ½z?ïôkâI¥?YH؄£?W)Ùü3åY?YH؄£?îò'|Œ?"±uSJG$? Öè4«Z?"±uSJG$?ïïUÚ>?PœÔd3?`ªæ,¡?PœÔd3?ïê¸cÅ]~?pŽâ·"ß$?eGœO@)ó?pŽâ·"ß$?ïÏPR*Å?ƒ5 C°n?xWðd©
Z?ƒ5 C°n?îÄM–r?¤÷ö»'?¨¾è'ãã?¤÷ö»'?ïêPYù_?^ׁE4Þ?eô¯fÍÐì?^ׁE4ÞAGN4FGL J0523.3-2527¿ÚÛL
ìõÀ=Ô2‡;ÉÀ9$éºC]MÀ<4x'@>^çÁð¦?ú[™hò1á?±
Á$"8?ÛE"~°	@)
fðÏáT?÷¡º¢¨¶î¿Í÷Pƒûø‰?£Drö—¡r¿ÔB©Þ5Tö¿âo9©nù³¿í隁öæ¿ïÿó5bBOTHERbin3FGL J0523.3-2528CRTS J052316.9-252737?s²õÆ£5?uÐgJÔ?ïØü™Õ9ê?uÐgJÔ?ÅòÔþõhø?ÀØB#Ža?êƒJÀB¥Â?ÀØB#Ža?©'?›{âü|¿?înfÞd?›{âü|¿?y€.¼ë~?qM«ï±x
?ïÌÿ¢<?qM«ï±x
?iÁbK$Ç°?g˜Ž7?ïæ>õsà?g˜Ž7?©¿7ô42?¨Ó¨e†?îd€°®M?¨Ó¨e†?ž³A0WþÈ?œ?aÁp`+?ï
eö˜¼ê?œ?aÁp`+?Ê1&R{H?<:»¨G?ïÿy®}èt?<:»¨GPSR4FGL J0524.4-2413?çø‹ ˜Í}À=3ÚÄç%À:©VI¸±À<:Ȇìî«@R`¤.É@`Eºõ4?Àuf3¦¿´ì×?}ªŒ?íB–%œr@¯p¢)‹¿Õ|qÀŒ¢¿èÒ±þ•FÏ¿äö©Àd¿êáÏ=jn´¿Üz¡Ü´ "¿ïÿ⾦™\OTHERglcNGC 1904?ïþD4üû­?&*«$Ö¤4?+¼³‡°°Ž?&*«$Ö¤4?ïõÔØßՓ?Z|‹üØð%?TVMÕ!
a?Z|‹üØð%?ï"0?Z~Ö¾ á£?a]mà€xS?Z~Ö¾ á£?ïüs…«›?%¯4 '-J?<cÓ©ÿQ?%¯4 '-J?ïþ=U ø?,I²ØÞ'?,*ªU·Êí?,I²ØÞ'?ïÖÃ7Å
®?{Ÿx3Ã?tžd7—°Þ?{Ÿx3Ã?ïÚw=VÖ.?w­oUø€í?rÄa?GU
?w­oUø€í?ïÖ.k´j<?jIUŽ›Çn?tèÊ#»6?jIUŽ›ÇnAGN4FGL J0524.7+4824¿Ú£èPû‰è@6D#EfÀ;š%FáeáÀ=G'u¦@ úèóžó¡?ý}ÒÉfÿ?ÛD^ÞÜ?ï¦jÍÔ3É@s''%Î@Ÿµ§ís¿éÆl`{jÚ¿ïÿâ¾÷!?ïþFŒ¬KM¿}87Sÿ0¢¿ì=˨	žå¿ïÿúâôOTHERsppSNR G159.6+07.3?ïÜ!2ÌþB?{íÂaù%?qïf·½n§?{íÂaù%?ï*Á,¹$,?ª°Gu©].?š§Úqr€r?ª°Gu©].?îv
ğèÏ?˜Røãeœe?¨Ÿ#¶ÝZ
?˜Røãeœe?ìÏ%²õ"É?¥Ê3Ù5
Û?¹†Òi<6?¥Ê3Ù5
Û?ï†WúV·Œ?"X?øŒšã?Žjx
?"X?øŒšã?í»‹lÐk?»5ÍÕر?²#¤œÛW$?»5ÍÕر?íHøéE?¦PFÛ¯ßC?µ¿€BwS?¦PFÛ¯ßC?çNÉÝë>c?À­Ì­BC?ÑblD)ƒ:?À­Ì­BCAGN4FGL J0524.8-6938¿è_†³bîbÀ@f>lLYuÀ:¯wOµóÀ<>¼(@ P&'º'.@#\ƪsÜ?Ƌ«Dfâ7¿q;ÞPÎg?»7…RdѼ@sÎáÏé7?îF7òµ•¿çM|5Om¿ëøýbô´¿×̤½äý¿Î±ZÖeQé¿ãòEÍiª¿OTHERsnr3FGL J0524.5-6937LMC SNR N 132D?ïü\£Z?3<›÷¼•?=ϵ³~?3<›÷¼•?ïöWÓ÷?VØz|Û	?SÛR^"??VØz|Û	?ïëù°'?c–Ѝ]ãk?dO÷ tË?c–Ѝ]ãk?ïüÐ^æ?"xšy&?9}%°Õ?"xšy&?ïõÓ`ÿc?Q´Q­Ô†?TàY:?Q´Q­Ô†?ïÚ¿åÄђ?zõBˆJò¯?r 

"?zõBˆJò¯?ïÜnH*Â?x(æñî?qÈÛþzc-?x(æñî?ïëŸ?˜=Æ?Xø¡a*?d`À')'?Xø¡a*AGN4FGL J0526.7+4254¿î_õç€á@<"Þ ²'À9¶5•
BßÀ;‰Ì·ÔD@r§qsŠ¼@'»0Ã?À=̀{æU?ÎÎ81ʨ@	Š]ò#žk?ûR-ÝZ¿ã>|b&:ҿфîê3¿çžfB)EI¿æ'¿BJ¨E¿ïþ&@Üi"¿ïÿ‡ÕK÷OOTHERsnr3FGL J0526.0+4253SNR G166.0+04.3?ìBm Ðì'?¹Ò°³Þáš?½ì–ùxžÅ?¹Ò°³Þáš?æô+±'<a?ÊmL-Cô»?Ò¨œÛ‡??ÊmL-Cô»?ì¨Ó›ž²?¤E2gšé²?º¹c#út?¤E2gšé²?ëmÿÚ7¼?k#³'?âH—!?k#³'?à :–
?Ê"3?߾ߊzÓí?Ê"3?Àx­VËúÑ?ÄtÉwû½?ëáÔªML?ÄtÉwû½?Ûz–Áon?»t¶Ø'—?âqB´ŸHI?»t¶Ø'—?Ð †Wó\?²Vy9uï%?çï¼ÔQÿ?²Vy9uï%MIXED4FGL J0528.3+1817?ŽÿÛ$ÐÛÀ"zd×ñÀ;
mzVÞ3À<bً÷ðg@""¦ö¤b?ù£l-Î?ÒêsÜp®¿?Ó<'`
ª@Å@Ìxé÷@Ug"xû¿¿ïÿúŒ"¸'¿ïϯ l²?ïÿõMõVY?_³nØ¿ÇÔñžé9À¿é÷ƒŸ‡DWOTHERunk3FGL J0528.3+18151RXS J052829.6+181657?ïò?ý¾S°? 0·RxW?[€¤1I? 0·RxW?ï냖Dqì?e½Y×õ8?d|i—Ò#ä?e½Y×õ8?ï¶ëÝðFá?~¨óñ5?'E"qÂ?~¨óñ5?ïÚÁ;7þ8?b¡íÊÏÊ?rŸb'=sß?b¡íÊÏÊ?ïú¤J]Ø?NÝå"ñÅ>?GámçðŒž?NÝå"ñÅ>?ÝË;?˜Û77"ƒð?ˆT9±I?˜Û77"ƒð?ï¶2\|5c?…/=~gna?'shìùI?…/=~gna?ïhæµùn
?ŒËœ'Û²?'ã)Eù¨[?ŒËœ'Û²AGN4FGL J0533.5+1449¿ß­¤%öÀ#•ÿ'+¾ËÀ:æí1Ç"iÀ<8|É:s@!M³ûo¢z?ø\'þ!?Ôèî Y'Â?Ùâwä"?þ ©¨ÛUý@_~ptZ¿çĀ}hák¿ìÃÏ,ù]O¿î—àÓ¿Û?èÙ¿y}¿æ©³ÊG¿ÐWÍÜÂ8IOTHERunk1RXS J053336.0+145115?ïü,-ÛZ"?ACê`œWÙ?>žÇ¶?ACê`œWÙ?ïñÔk]"?\¦"žhÀô?\WËGhß?\¦"žhÀô?ï±.\oþ§?€"d2ïhq?ƒ´hÜÉ(W?€"d2ïhq?ïölGÉ9½?DUÛËr2H?S'p1fñ?DUÛËr2H?ïûCí+?FaÝðÍ´?BðJ¬Ì÷j?FaÝðÍ´?ï¾A-g—?Šò}¡Æƒ?€o¸{…R'?Šò}¡Æƒ?ï†ì¼4ì?''‡"?ŽDÐùÞüñ?''‡"?ïË-Q‹§­?u|¹ºMz¦?ziWŸ……?u|¹ºMz¦AGN4FGL J0534.5+2201s¿æDùQ:/QÀ 6m
JÀ6"UõÕړÀ8{•É*€Ý@e
'àÃ@
Ÿ²$ªÚ4?Ð^beOæ?åLïg+ˆD?÷±ÇÞP'Ï@ î'š!¿ãq9"Ÿ"•¿í¦È •¡½¿ï·Á½ob¿ê tοêÑ¢ßé_*¿ï
²¢\·OTHERPWN3FGL J0534.5+2201sCrab Nebula?êÎ$óvÒ?ΪÃqžÆ?ÄÇl2$·½?ΪÃqžÆ?ïôB"èœ?aT¨äî?WzØY
á?aT¨äî?䔰¨Ì3í?²¦&̛Å0?Ö֞®g˜&?²¦&̛Å0?ïÿ›T•êŸ?<yëÖpS?	*äP;G¥?<yëÖpS?ïÇÛÐ#l?•±‹gw"~?|œö?•±‹gw"~?ï¿Óa"?'âßèñ62?€°é+"?'âßèñ62?éßÉÕ)EQ?¯9Ïô8ef?ȀثZê»?¯9Ïô8ef?ïþ9Ü/Ë?-žÁ	äí8?,b>OK?-žÁ	äí8AGN4FGL J0535.2-6736?їޒ‹ÍÀ@óGÀ9[‹]–´À;«qóbbÌ@<°®;Ž@ÅÊz5˜?µ	5'?ÈŸ‰ɺ@d:æ…Û?ý˜ä«㣿©òÕÊø6]¿ç$²1@ì¿æ¥Õ|ž·¿ëP™àç6¿ìC‡¿&›ö¿ï^²"&›uOTHERHMBLMC P3?ízâõ¶®†?´*óœwøé?´(èR¸P?´*óœwøé?ë'ì›
&?Áloû÷˜ä?É´M"Ëh?Áloû÷˜ä?ìdK ºµž?¤Á5ãéSS?¼Ý¦ú*S?¤Á5ãéSS?êÈpËUd?¡ç'Œ£÷G?ÄÞ<ÒªmŽ?¡ç'Œ£÷G?Û¯•97¯?Èc›çÔ?â(5cd(t?Èc›çÔ?ÔÀá¢ÐX?Ñ>»ÏEðG?åŸø.—Ô?Ñ>»ÏEðG?ߺ—zmî?¸*gM¨:­?à"´BðÉ	?¸*gM¨:­?ÇÚAgï—?±lg)?ê	o¹æ?±lg)MIXED4FGL J0537.8-6909¿ïõ!È°;$À?¾)Çy¦µÀ8ÿ[zz¢À;b8¦@!&±ú8•É@Dº"»äG?®!ý"L}~¿œÝÑ_Œ?òˆêõ¬À?þk,kÃÈl¿ïü,k˜ÕN?ïF2nè¿ÛU^–cY¿â/Ljp|¿åðª!§µ¿È÷gjW¿OTHERpwn0FGL J0538.4-6856N 157B?ïô
VˆV?'©Þ5dm?WÙå,sµ1?'©Þ5dm?ïÛ\	k8³?ƒvjl÷?rQû_NQ?ƒvjl÷?ï^Â×ð0C?ù»¸ëRü?"'¥i"›?ù»¸ëRü?ïâ'm?Œ%Ճ}ï?œÝŽGNY?Œ%Ճ}ï?ïÛŽ•&?m%ª áb?r|wRÒtÔ?m%ª áb?ï\@Šß—€?ªÞÞIb?"wîªìGÿ?ªÞÞIb?îùJªø?˜æuZï¤? k_÷Þ?˜æuZï¤?ëKê[ \#?µ©áyñ?ÂÐV'~t?µ©áyñAGN4FGL J0540.3+2756e¿ØúLö‰¿÷ÿ@wÏDÀ7˜€dÀ:nÔw»ù@@ƒw3@$Ñ~uY?©f\^rT?¿úBPÝh&@•èO	R?þ`4:Å"ß¿ä7Ö ²Q¿Ò¯&ÿHJ¿ÞÐÏ%l¡¿âí±^\Vÿæ²Ô~«¿å¬Xž&ÇOTHERSNR3FGL J0540.3+2756eSim 147?é™ÉÒR?ƙéˆøÀ#?ɘ۰·º¹?ƙéˆøÀ#?×ÚÓ÷Ÿšv?ɍ(¿^Fª?ä–02Å?ɍ(¿^Fª?åwX<¾2'?´2±«w?ÕO†ƒšÝ?´2±«w?ãC¸U`I?¬ßkÅQׄ?ÙõxU?o?¬ßkÅQׄ?âo{—[?ÌæýÐ{?Û!ÑéIä?ÌæýÐ{?¢4Ž~½³?«®oøðÉ?îÞ¼·3'?«®oøðÉ?çÔÁÛ­m?²Çtq®Ê?ÐV|H¥á&?²Çtq®Ê?µ;¨Tuâ«? 1¤¢=*y?íXŠõUÆË? 1¤¢=*yMIXED4FGL J0608.6+1149¿íhtÛʸÀEà.©`·À:5.¬À;´¦Hԅ(@s¿®+L	@M»$-ܲ?Á™UQF¿›'ý\ÑV
?Ú³Z€)0%@eZwÅ´¿ßWú'ص8¿á˜f~9@é¿ê˜!"¥>¿×mÁðzÒ¿å'U¢ÉÄ¿ÛöUDz±™OTHERunkNVSS J060835+114942?ïýãKµ?&··ù,ÊÒ?0姗S¬?&··ù,ÊÒ?ïðG]·–/?kÌa·'ç?_qD>]Æ?kÌa·'ç?ïӝ©s¬J?€-2|Ôe?v1+I™vë?€-2|Ôe?ïûäL›9,?&hKuñØC?@nÎU¸bc?&hKuñØC?ïó¬TÝ'
?^@•´l4°?X§V"êµ"?^@•´l4°?ïãÑÝ>?›~qÚiÁ°?ˆ‡zò	~?›~qÚiÁ°?ïaÑx?"Ã›ÅÂ?"ß¾…Ðþ¤?"Ã›ÅÂ?ïå¶.¿tä?]êÛ¨E?jIѯ£ð?]êÛ¨EAGN4FGL J0608.8+2034c?ÉJ…ñWVå?֒*߈'À9Û©ßaûÀ:ɛëƒq9@™ðX˜—@"‡vf?Æ~ÿyó6?ÆûBÁp£+@0¦ždÚu@@®pì&¿ïÃvõ׈?ïÊÁ$"8¿èË[þ®qB¿åµ¦	êd¿ê°Ì†Uï÷¿ïÿÿ&¦³OTHERunk2FGL J0608.3+2037NVSS J060900+203746?픹¼én³?µmËF8>M?³Z2´Ši?µmËF8>M?éFCÖ;?Çö`Þ«á?Êæð§÷ü?Çö`Þ«á?éÙÎ:铋?±¾ôÞ>R?ȘÇY±Ö?±¾ôÞ>R?éŒÝñ¸> ?ª?y¶jÖ?É̈9?ª?y¶jÖ?Ú@A9ÂTµ?ËnetŠ'?âßßcÕ¦?ËnetŠ'?֗"èœY?Óÿê.e Ê?ä´n‹ñ1Ó?Óÿê.e Ê?Ûø
;ï<?ºôj­jSR?âúâpb?ºôj­jSR?ÇÐúó•}?µ«%žzGý?ê9ÁC¡?µ«%žzGý$MIXED4FGL J0617.2+2234e?ë>éÆò\@DÚ`3FÀ5†õ)iÀ9ƒ~mÄ(¹@ —r،I@ýo¿«|?‹¼ê	Q@?À>¯þŠßí@6ú;šàÁ@$&žü?îxˆr)é¿ÐPF~êkÄ¿á_eÁ$øÞ¿áÅÞ,ñ{¿æ*Þ)£¿åWǂ
0ÛOTHERSNR3FGL J0617.2+2234eIC 443?»JT!•Q?Ço¦t& .?억{ÍUß?Ço¦t& .?§Éű-›?¥RÄ£&™?îƒc®"í&?¥RÄ£&™?áÃç§ÞD³?³¡²r¼À?Üx0°Cvš?³¡²r¼À>ás9VÜü<>åöx|Oì?ïÿwÙ>åöx|Oì?é¹l¸?Æ$núat?ë'¤Ø'ý?Æ$núat?z£U¾!0 ?€'Woj?ïʹTJ0?€'Woj?èãùÒ>{¼?±›¢ljÑ?Ìp·?±›¢ljÑ>$c.â¼Ú»>Hr"¥ã=?ïÿÿþíA>Hr"¥ã=MIXED4FGL J0618.1+7819¿ê¬4M(kž@8ݘ9GIkÀ;#''Œ6À<ÎYáÒ@Lû°>@D.ÛµÜ?ÀY3¢ï®¤¿µ;Šo°*?ð¦ªú-´?ô'ëí¤]Ã?ë8Åû!?¢‰grU¿å]Ðà؝f¿ÓÛ\Ý{›­¿ìÛ~WžÍ?Øý¥²¬OTHERsbg3FGL J0618.0+7819NGC 2146?ï鰚‰{?p«M)‹5?fOe1ÌŅ?p«M)‹5?ïw‰¾§'x?—÷.ˆ7¶?'È.}Lú?—÷.ˆ7¶?ïoËV¢pz?‹WØðKËé?'•(BT¾?‹WØðKËé?ï×ÃBVß?'kû•#öz?ŸÅ•ýV"?'kû•#öz?ï®·Ì?ÉécH‰8?"RõŒ±?ÉécH‰8?êÁõcþÿ?Ç5lÑíü{?Äø*sœ?Ç5lÑíü{?ï˜C 56?‰`±"¹À>?‰ïý/ñ?‰`±"¹À>?è(""±ð?´'ÏQµ ?Ï]­®8B?´'ÏQµ AGN4FGL J0632.8+0550¿ÄÀ¬ÖÀÊ¿÷*°ãb:ˆÀ:b›!YÀ:ý³çùxý@!Ï¿4ïc@%!š"{$?À'¬î
46¿¸?³ÊnK@üR`õä@>bq`?í²µ)B©¿åèÍÿ|Í[¿í̌€V|Ž¿Ù÷›Â響à³Ü:þُ¿ß÷ë>Qõ@OTHERhmbHESS J0632+057?ïâ¼!Ȗ?'t|ðÇù?màC×X1"?'t|ðÇù?ïc-ãNT³?£L16"?"šC"}›¤?£L16"?îò°ø
 Û?—Å(}GŠ? Ôð%òO?—Å(}GŠ?ïǯpÌq?srV`>=?|(z/Œƒ³?srV`>=?ïfe´²=?•ö]™À?"3Ii¼˜]?•ö]™À?ë
ßv¿ò@?Éð-´ï?ÃԂ%6ÿ?Éð-´ï?íË^ÄAÊ?£Ž_ @Ö?±§•¿­?£Ž_ @Ö?ëó:®7òq?·j¢¸H¨³?À3G 6=?·j¢¸H¨³AGN4FGL J0634.2+0436e?ì†÷Xű¿û4ÂI¼´À7cx WÀ:]I.G;(@	G&…%@Ôó\ƒŽ•?§'/ÞêÝ?ͯº'ÈFÖ@"×\l¡?øá@âV¿Ô(þ;"»f¿Î…:¼êV ¿â†HÿxE·¿ç"O…yQ¿åYÏ^ø]õ¿èxŸN€ÌOTHERsnr3FGL J0634.1+0424Rosette?ªD}†´&È?µÕW'ÿo¹?î[¸'y@´?µÕW'ÿo¹?²EŒ¼©Ð?®²Ê'š¤‡?í·N€
"ö?®²Ê'š¤‡?Ö%Ç-r÷?³ ››-k¿?äíqœiF"?³ ››-k¿?—…lÎÐ×?…81?€-?ïCԙR‡?…81?€-?š¾Jù¯v(?™yìi~ñ?ï*
¨	Hÿ?™yìi~ñ?"šY0h•¥?‰dVÝ*"³?ﭖ›Yډ?‰dVÝ*"³?Þ.Aٌ?·§y8ø…g?àèöøß:?·§y8ø…g?+æõ¦j?$M*Ü#–?ïþAž}P…?$M*Ü#–PSR4FGL J0639.4+0655e¿×bN
?àŸS À7 /^'\ŽÀ9À¡²lÏ6@o½fþ;Û@a&Á4é?´b_£ÿ?ÏÆæxFä@X_^4h½@@í°òý?ïÚ䜸2¿× (ú¿åcÀEç¿äŠ]âsA¿ëÉF/9Ä¿æJe~ßÙðOTHERSNR3FGL J0640.9+0752Monoceros?µ›€R	ˆ?ÀÇ9¬L­?í]¬ÚAï?ÀÇ9¬L­?·g7(?¢?²Ên±Î«?íêML?²Ên±Î«?҈–:òù?±–þ¬ëFe?æ»þ´â†"?±–þ¬ëFe?¿w¢£Ùc‰?¡vsËdþî?ì«"ӏ?¡vsËdþî?ƒ‡Ž©¸D?§ñ•¹M.«?ï±áÇä8W?§ñ•¹M.«?†{ü2'¿?ŠŽc¿ôËd?ï¦l¯?ŠŽc¿ôËd?«[
ñ(T?®·-(W7?ëU)=Cµë?®·-(W7?lºÙ—Ïק?YÕ"δˆ?ïãE&G3é?YÕ"δˆPSR4FGL J0647.7+0031¿snŒ"™¿âN»ßê‹ÐÀ9p°;œŽAÀ;X4Ò@ŸÕŒcûþ@ÀùÅS[È?⡟øXkÒ?ÃÆe¿øS
?ÿ€–"TÜ@‡f$w-´?ïÿhJí¿º¯÷¤ç«¿éºÄöJ¿êÒêRï'¿ä

ù½Ç¿áÓàx"OTHERspp3FGL J0647.6+0032SNR G213.0-00.6?ï¢%ëæ²@?¦úµDCF"?‡v"ÿt8
?¦úµDCF"?ï~Oþ½W0?"t°þ{u¶?6#-¯û?"t°þ{u¶?îÄeûåò–?—A#ñ'É=?£¹ Er—?—A#ñ'É=?ï5ÒE˜Ì¦?yêµhF®B?™E·Nž95?yêµhF®B?ì-œµÄñ?¡k¢1åù?¾"W!Øv?¡k¢1åù?ꠁ¯?Ç_@¢‡~å?ÇÝ}ùCçû?Ç_@¢‡~å?è´ðrCia?³"mí¹î?Í,>6òZ{?³"mí¹î?ç狼%#•?´bÙf¿¼?Ð0臵¸Ö?´bÙf¿¼AGN4FGL J0650.6+2055?çø×:ËJ@"h/"BAÄÀ9æۚÅé"À< öðŒÅ@ úe	.O?û

jKÎ5?¼a%r†Û?³d' +C¦?ûVʗhfò@VX§6?ïðHgwÞ^¿æ¨
/"k'¿Ó6@®ÆÒ¿Öµ@S­&>¿ÖasÕB<¿Þ·a`m("OTHERunk3FGL J0650.5+2055NVSS J065035+205556?ïû*ÈwõÒ?5Y®àK'?CTß&ñ;É?5Y®àK'?ïå!
¢×l?p•=uÁu?jÞõ…ª?p•=uÁu?ïëìêq¶?a÷CQd$Û?dÛ°Q®?a÷CQd$Û?ïÌÛ>ÄO¿?[¯¾À¸Ì?y'`ƒ»j?[¯¾À¸Ì?ïñ]S©[•?PŸîŠÚÇ?]EXª‰&•?PŸîŠÚÇ?ï]
±x¢B?œ'Zfýæ?"^©Í|Æ?œ'Zfýæ?ïÎ`½ñò?€Ê!ùd«?xÏ¡‰JÂ?€Ê!ùd«?ïUý"" ¨?~²"v	?•@Mm´?~²"v	AGN4FGL J0709.7-3009¿ïë½>ÿ"À#J½ÂmÎ:À:—¥ßøù|À<b+¡ƒs@ Šý?ÿGKƒŒ?ÁY:?w9gïlMË?¹Q8½òÐ~@F¸4Õ?ïÿК·¦Ë¿éiüp¿Ô/(âwXý¿ãŽþ "of¿ÕŸ{¿ßއŸÇ8OTHERunk1RXS J070947.9-300901?ïý¼Üó>.?%¸±©Z'Ñ?2DP"?%¸±©Z'Ñ?ïô û
?[{'ÏHA?V¿Ññ2µo?[{'ÏHA?ïôe^˜U'?Z÷YÎâ?W5BEä‹?Z÷YÎâ?ïü2`Øæi?$}Á¢Œïè?>lúOà?$}Á¢Œïè?ïý}I+íð?0ž/yÝX?4¸4ÔÉ?0ž/yÝX?ïÒekGT[?"LÜ/Hö?vÍJN—b"?"LÜ/Hö?ïõ¹>
ãÅ?c}Âu?Tƒ'Bv–?c}Âu?ïõêÙ/å)?CƂ²Lé?T*MÜ®Î~?CƂ²LéAGN4FGL J0744.0-2525¿ëJ¯×|0Ü¿ç§ÃÉfÀ8Ï}ÓjuÀÀ;z鳍a@Š9-s*Å@¡½aõ¾^?³ÝLvѵ?Úͳ\cX?@#HÈ/ù?ÿŸlÊX©9?äJSá)¿ÓI }8é¿ÜY"åO¥…¿åßÖÊ|t¿ð?ïÿÑqw;¡OTHERbin3FGL J0744.1-25231FGL J0744.1-2523?Dá¦ZÞÿ?SRìNƒÙÜ?ïúǖyv?SRìNƒÙÜ?²¹ƒò_Ñ?­«\îü4?í¨Ý/´?­«\îü4?®Gl͟
? (ð"<?î{‰@ä? (ð"<?¯õ"²ôâÕ?ž¯™D»ïû?«'?ž¯™D»ïû?xC­¥ÿQY?®•Ѥaš?ïÏx¤½ E?®•Ѥaš?'æ1®PÖ?…y ÞeC?ï´g:C?<?…y ÞeC?™‡kˆ~(?™rÚPuv?ï3Ä£¼ï?™rÚPuv?Jx…׈'ò?DؕôSJ!?ïùaÞÊÙ¶?DؕôSJ!PSR4FGL J0809.5-4714?ØéՉðëÀd]wª\À:
%ÍïâÀ;ÏVØSéŒ@Á…§IZ'@*N뒋?Ã'CeÛQ?ºH"Cnj?õS½vd?ýŖ­V¿ÙT:귙¿×ä[Ê+1Ý¿çý'1ÆK©¿åÈØ\œ8¿ãف±E‡Ê¿ïÿîÝÃÀ	OTHERunkGamma02 Velorum?ïöäu,tJ?DóޡϽ‡?R7Ól'?DóޡϽ‡?ïÌÐTZ?"6ÓgÏÔµ?y—Õ¹K`à?"6ÓgÏÔµ?︰}?{Nã­®ãO?à8û¤D¦?{Nã­®ãO?ï±Ée±'?d5a¿N/?ƒ¦ˆø²
?d5a¿N/?ïàî‰ØRß?cÝÝ>ª¢»?ov-,€¶?cÝÝ>ª¢»?î¿Â3´7?°òÕ¡Â?¤ÞÛîŠ?°òÕ¡Â?îۂ´>¥F?™\¯6›?¢GÔº]Ý¡?™\¯6›?ìýôãY›?¢1£ÌY|¡?¸_&?¢1£ÌY|¡AGN4FGL J0816.0-2342?ÍNâÏv(@o4þåMÍÀ:SŠ ÒHÀ;Þ€@J‹¿f\Ö@–Ÿ¸g?ШÄûb?Ó.ƒ€Óz@¡zSƒ5@ˆ`â¿ßRBã)…Š¿ç±/Lô¥Y¿èђ>†x€¿ï[nÎ?¿ïu'>³D¿ïªáö)½iOTHERunkAT20G J081524-233846?ïç@;·ï¤?eó1ÚPj'?h¿Äzê"?eó1ÚPj'?í
rn´?»¼î"Úß?·"oÛê}á?»¼î"Úß?~°?"|q"ƒ›?¥Åç¥cú?"|q"ƒ›?î}­SF	`?Š{¤ª?¨%*˟j?Š{¤ª?ïËüDð±?~òiƘ'O?z~ÃjŸš?~òiƘ'O?؅†Ñ"±D?Ó4zöÁ<÷?ã½<—=§^?Ó4zöÁ<÷?çn"½Q?µ+ù ³kâ?Ñ#Æ؅×_?µ+ù ³kâ?ßÖY&ü‡ê?½IºøÓª¦?àÓl¼?½IºøÓª¦MIXED4FGL J0819.5-3439¿Õ9–Т«w?ëû=#JÀ9ÕÊÛ[	À;zºÖ*D@ég)ÚÄÝ@":ÚÇa?ÎTð]-Ù?Ø"Ÿ€&@þ'Z·Ü{@¼L0Z;?ëˆÒ!Š_¿Õ(,ÚSž
¿êÒiY_í¦¿èÓÀ§$œ—¿ïþP¤]B¿¤­ÝTOTHERunkNVSS J081945-344215?ïnñT8ü?!Ì&¶W}?'!ÕwG2?!Ì&¶W}?ìã2V‹ÊF?ºÛü>¢?¸æmMY{Ò?ºÛü>¢?íę³'½?šÏÖ0g•ª?±Û3'cr?šÏÖ0g•ª?헫ðUµa?w‰A¹‡?³B {š†þ?w‰A¹‡?é|{é&ìö?ÁÊíy•˜-?Ê[dL'?ÁÊíy•˜-?Ñ[Ò§?ÐJ¨±JÌh?çR@ùõ-?ÐJ¨±JÌh?âh­ö?YT?¹%näåz?Û.¤MY?¹%näåz?ڝª…z'ä?³]畧¦à?â±*½Bì?³]畧¦àMIXED4FGL J0822.1-4253e¿ìè»Z+À
þ€{»bAÀ7M—üágÀ:ª}ÞR0N@ƒexy?þ"Á-\Y?Ñ÷À&²X?¹Í½7®m@Ìx £
·@XðCõMJ¿Åi€Íú¿Ògáæl¿Þ=êg9 ¿Ü­¤"r¹¿äŠS«x¿.¿âgk*NOTHERSNR3FGL J0822.6-4250ePuppis A?å'l³ÔП?Ê¡
vÚA?Ôû&˜V^Ã?Ê¡
vÚA?ЉT1ÛoR?ľn•f?ç»UçHW?ľn•f?éMõ‰âö?°0â_R˜?ËâÈ)Øt(?°0â_R˜?ßueú¨º?³SN
€à±?àEM«ð£?³SN
€à±?ç!ÄPQ|?ÇAéCûØS?Ѽw_]Ã?ÇAéCûØS?š´ð
ùÑ?¡×қ`³?ï/
XN¡?¡×қ`³?ì""Ôb»?ªï¸ÞN?¿fé\ê+?ªï¸ÞN?¬ùn°%¼?šI
ï?î>iYµÔ?šI
ïMIXED4FGL J0833.1-4511e?ëa…DçªÀÙ0¾
í)À6¿Þ^sSÀ9BY`Äeö@!ägÀ`@QŠ¡¯Ñ?¦¤©;?¡ÙÖ~/
'?ô,Áÿê1@ãhšž&q?æU€e.?ҩ… ¿à8¸¾M<¿Þ¾u5¬¿ç=ñ7¿âµÚPp[OTHERPWN3FGL J0833.1-4511eVela X?àuzqúÝñ?Ôd'¿h?ß
D?Ôd'¿h?î0ˌ°Òñ?¿²3Հ·?¬óG7†…ê?¿²3Հ·?ä&#y=î?³Ù"`;Ð?׳¹
…Ø$?³Ù"`;Ð?épÕç8ïò?¼s6ñÑ?Ê<¨c@9?¼s6ñÑ?æD5A*l»?Î,Xz·Î…?Ów•}«&Š?Î,Xz·Î…?ìÎƇA?əãÔ®Ì?¹ñÊ|Y?əãÔ®Ì?èk©Û,?¶" öa?ÎQ[ГßN?¶" öa?Þ/°¬Û•½?ȝ(Suß?àè'©'5!?ȝ(SußMIXED4FGL J0838.7-2827?çMàØ8ç@=5¤&»À9"©¥€W©À<pÛs@Í(+˜4??þv9ïå×?³€šëSK?Ó3\£Äì@ïbùÊ\@$ïªGfÇ?ïõT9¿¯ÏÛ Ñ¿Ü{ÔA‹:±¿ÞœÆtÃ÷;¿í­òˆH8¿ïâ."'AÜOTHERbin3FGL J0838.8-2829XMMU J083850.3-282756?Ÿo/øÔ?¬ÃæZx­¢? ©?¬ÃæZx­¢?»ÜgØ?µo²	š?을sdþ?µo²	š?ÃV;I?¯nI ê¸?ë*}ñ-»`?¯nI ê¸?Î	Úi˜u?°5Ht–ˆv?è}‰e™âÀ?°5Ht–ˆv?m7Â.Ñ3@?kqÃñ·?ïâÈ=µ±í?kqÃñ·?‹Àq÷H‰L?
¿ ?ïþ8`û?
¿ ?œ  !±¦?"y7ë¶?ïþÿ°ã?"y7ë¶?ŽP/"Ùp"?|Q'‡šE>?AžÛÎ?|Q'‡šE>PSR4FGL J0851.9-4620e¿æÚÉHº{¿ó·þ½à¡À6Õ6$;JÀ:p³"&k@!²KH¨»K?üßѧ' Ö?'Jf¢î¤Z¿"¿g€å?ûÄ¿9aK@:=,0_™?ï	H]ç¼½¿Ö©CEO¿âm)c¦˜†¿Ûd`½/þ¿Û±€@,?ú¿È ƒxÅäOTHERSNR3FGL J0852.7-4631eRX J0852.0-4622?î!î‹I°ß?¶ÞZæ®ßÍ?­áI­$?¶ÞZæ®ßÍ?ïŠk•ò'|?©Êvœ™-?eƒ[a?©Êvœ™-?鸐Þ<¿?²a¥UV`?˕¼‡
?²a¥UV`?íµ1ƒÁÒ.?¨>ÖÌÍE?²Vsâ_b?¨>ÖÌÍE?î¥
"^/F?°…¨(¡¶?¥¯'»Ôٖ?°…¨(¡¶?î®ÎÓî?´kH´?¥Ò »æ?´kH´?êÎlªÖ¶c?´Ë*»^s$?ÄÆMT¥&s?´Ë*»^s$?éÉð‰•j‹?À‹ò£1Y?ÈØ=ÙªUÔ?À‹ò£1YAGN4FGL J0852.5-3123¿îƒ$Bˆp@ ½óùa€NÀ;,%5À<ƒ·'¸¬"@">NÃ9%?ö.­ýÔ¬•?ÑàÙ^«‡?ÏÈžžç?ôŠB®Ñ9C@2õ#Øø)?ïf¿2Zp¿ïÿQ^ÂX*?ïüÉÚ¨X¿Ùoß¡eÀÏ¿Èø»h {¿Ð$—Žý^OTHERunkNVSS J085238-312331?ïúöp+®|?6'ünט‹?D&?®»o¥?6'ünט‹?ïæKaä\È?tlLjÄ?i´ž#âHb?tlLjÄ?ïÝ0Ø:L?q˜
áh²ë?qg"Ïž?q˜
áh²ë?ïñ˜r
tÄ?I"bïœ,1?\Ï°ÜhŽ?I"bïœ,1?ïüXˋ?<ûae»á?=?/¥j ?<ûae»á?ï=fk!"®?¥
³ØÍ?˜S2"î2O?¥
³ØÍ?ïÞN9lÆ?xc	Íѵ
?pØãTM]?xc	Íѵ
?ïæ•^ ?b(±ǘ?iìj¥þëM?b(±ǘAGN4FGL J0858.0-3130¿Ûß÷ªy™@"dj ‡ÊdÀ:^Y­ñ?sÀ<6×%ì"Ó@!±Ÿˆñ֝?úÍwҟt¥?ÃñîšQûJ?·ø™Àl''?öf2ƒ
@!Uå?ïâO`:}T¿ìénù²Þå?'îSžýJˆ¿Ñ«ýI2¿Ôž[JS‹¿ØUd.(OTHERunk3FGL J0858.1-3130NVSS J085802-313040?ïþÂ0o<,?¶¸›mýÊ?#ÜùˍìÝ?¶¸›mýÊ?ïço…žåß?t@tßWîC?hz y˜?t@tßWîC?ïùóêH?Uwn^?Kà0µûvˆ?Uwn^?ïõ©–ƒ?;RÈâø^?T­ý	ó¢8?;RÈâø^?ïþ¨&VE?)Ç˜à˜·?%~{ÈjO?)Ç˜à˜·?ïJÝüÊìM?¢¯®"Ѐ?–¤@kÉà[?¢¯®"Ѐ?ïù굞'?^Ô«4§?HU(á]u×?^Ô«4§?ïäãéì9Ç?ZÒp‹'t©?kH)?ZÒp‹'t©AGN4FGL J0904.7-4908c?íŽÊí	êK¿öú@óæJÀ8ÖÞZ"ÊÀ:Z¿»lR9@\´5ý@	STÛúg:?Ð@rM'À?ß݊àY@ŸÖjÛ@@j>NX(¿ìîàwW?ÛO®~ƒÄ¿ëU£ ƒ˜¦¿êÐäôá¾Ì¿êž–Xœy¿ïÿG]â‰MOTHERunk3FGL J0905.6-49171RXS J090505.3-490324?æº{<?Òî¾jšŽÈ?Óü‹ã߉?Òî¾jšŽÈ?ÕêD–KË?ÌÉ+³ô?å
Ý´Úq?ÌÉ+³ô?â̜Dž?³ŠkË4"2?ÚfÇÇvÃù?³ŠkË4"2?Ý%L$ñ¦÷?¶;QÊ)?ámYí‡,…?¶;QÊ)?äAÕ®%uc?Ò ÑÉXE‰?×|T£µ:?Ò ÑÉXE‰? Ô$qð?®`¨²øK'?îò·îvô1?®`¨²øK'?Õ¡–÷Ž?¶qµeW;´?å/4"}8÷?¶qµeW;´?ˆâˆuÚ͖?"C"‹«Ê?ïœuÝãܚ?"C"‹«Ê4MIXED4FGL J0910.0+4257¿åpîÈ}»@EvFbºà;À:i—Sn<À<{8bG@è!©s~@<¡pþp?ÎêÒñ±‰?ÓЧ¸@MÎ@5@%Nn@·'ŒYë?íݻŽZv¿äðÄ"ð¿äÅõãF‹Ö¿ìÒÏæ\ÀË¿ïì¿EûŒÔ?ï¦ë\ÕOTHERcss3C 216?ïãÃ)Ç	û?¢ÂBzæà{?l<Õü|äì?¢ÂBzæà{?ïÛV¡]™t?v^™]ʎ—?rT¯i@‰©?v^™]ʎ—?ïg(†d'-?†Pã-ƒD?"ï/þ>m?†Pã-ƒD?ïfQÄ©ùÊ?{K£`"š¬?"5ÇqŸþ®?{K£`"š¬?ïÒˆ4?t™_WÁlx?vð;ÞȸÄ?t™_WÁlx?#™|?­ö̚_ا?¦÷mÆh?ì?­ö̚_ا?ìä9Óçƒ?¦%'UÙ?¸Þ1i¨'ä?¦%'UÙ?ëUî$œ}¶?® ÆuÏøÂ?¨GmŽ	)?® ÆuÏøÂAGN4FGL J0912.1-6449?êò\QBE}À&n8§ç:6À:œJNìÀ<=²ôݍ@u±ô¯>ò@‡È
±™?ãHv;?Ê#ðõöç¨@æ;ƒcÍ/@)åËv`"?ï^·E|¿ÃjÓÞcøù¿ãíŸ
⵿ä`³Ô®Bž¿ìª0À',¿ïè,9CîlOTHERglc3FGL J0912.2-6452NGC 2808?ïvL[	n?'/ŸEy2¦?'6t¨•Ø;?'/ŸEy2¦?ï£D¢58`?…Ú±~ø	?‡.×aƒÜ!?…Ú±~ø	?îýçê_"Ë?"»ZÚM0? !WsþV?"»ZÚM0?îáÔ=ÚV"?€ÔhÜê$—?¡â¼!~¶Ü?€ÔhÜê$—?é*Ù,#ü?¿Ï°†3úó?ËT›Os¨?¿Ï°†3úó?î'NØfo1?­uý&>«?§Ûx½%ò?­uý&>«?æäPÎR?¶n=ƒÞ9?Ò7û_îc\?¶n=ƒÞ9?êôÈ?¦5>Ôrt?ÇÜ/‹ˆß¸?¦5>ÔrtAGN4FGL J0921.7-6317?áø䞶ËÀ"Í$žDúÀ:÷I,™»þÀ<¨p˜ïO¯@µÃvâµl@oÿ^ðP`?ÍbvAЯÛ?àÆýòÿf@}ñ'Ž»?ïþޔY#¿ïýSõËÊ?ïÿ¢­>'¿Ø†±_ˆü"¿áÔêp6Ê¿ïÿâÙ~‹÷¿¹à—/'âOTHERlmb2S 0921-630?éH!x`?Ãõ
£ÇðÅ?Êß{þ¢?Ãõ
£ÇðÅ?Ú{‹~EL³?ÌÊùDòDÎ?âÂ:@ÝY§?ÌÊùDòDÎ?æ‰Ïr?²é'löð¯?ÓíÔaõ?²é'löð¯?àý⌅<ž?±A"¸Zæ0?Þ:æõ†Ä?±A"¸Zæ0?àûãveµ?ɓh‰ùŠè?Þ95֕?ɓh‰ùŠè?³q©—fÚ?¼¹(™†?íÑʖe?¼¹(™†?Çc''Æ?´ù¡â¦b?ê':úÛ[Ž?´ù¡â¦b?­à§Ý»?—Òy
"Ö?î!õ'<t"?—Òy
"ÖMIXED4FGL J0935.3+0901?¸&S%ìΠ@D1'€w‰¤À:&<ì™.À<‰w¦×@	ÌžT@êû܄е?Åˆ¤~Ïê?Ӌ'Û9w@
¸«ôÌ@Ûa:,¢¿èÌ~=šZ¿Ð§ýàk¿ãèÖt¿ëp×£Àd	¿é g´D?Ë¿ïü²ÙÀ3OTHERbin3FGL J0935.2+09034FGL J0935.3+0901?ï1ÝXòF? â4¿¯–?žÄOºMO? â4¿¯–?ïÕé3¾Q?"">=¨W"?Š…¯ ÏÀ?"">=¨W"?îmô÷R M?™s"4—1A?© °ŠÝû/?™s"4—1A?ïmÓÝÁ?sòt®S?'\/Ê«±à?sòt®S?çl†§??ƃ.™×"6?Ñ'Æò±ý'?ƃ.™×"6?ëô^ÿ"Ë)?ÀÀÐ?Hl?À."¬Ó]?ÀÀÐ?Hl?ÞÁ݅à2?ÁJÔÍÕ¾ì?àŸv'=ç?ÁJÔÍÕ¾ì?ëX"h?©DYê4Å7?‰ï"²`?©DYê4Å7MIXED4FGL J0951.7-5328¿ª{ø.[zS?àœ2#iÀ:,F)¯ü²À;€U&£ø@ *úõÿöñ@Ï=ÀTïF?»•«ß}´¿·tA4A•?ùÑ(çÖz@o…'Ñ~b¿ïÿKâCW?ïø›AåR«¿èí][zпÜÅåNë ¿æ—â?$Øý¿ßFôçôOTHERsppSNR G279.0+01.1?ï÷ÝÚf=w?H¶èLæËç?PDK6W§?H¶èLæËç?ï¬ÚvÙ?0±ö-V?"û¹ZU‰?0±ö-V?ï¶ðBë?ƒ›9*F?'yÞÇ3?ƒ›9*F?ïÓô¦Ûv‰?agLa
—?v¬qH{Ê?agLa
—?ïÙŽ•žQ?q2ð½È›?sr8"4—š?q2ð½È›?ìŠ`QàƒŸ?Âø0Ó²o?»¬ýpûã?Âø0Ó²o?îžìÏC"?æ͎o˜4?¦3
†kã?æ͎o˜4?íúºxâ>ú?¢Èío‡?°*,9[û°?¢Èío‡AGN4FGL J0955.3-3949?ïGäΩÏ@'ì9yžRÀ93"P>ÝÀ;¦d—YMy@³›­E@óþ?¶=̀{æU?Ñ¥«`@‡…@ñ'©"á@THV±?íêhô¶â¿ÜÞdå1óm¿ä†2Ÿ£‡¿æÆŠÁX¿î¬­½½æ*¿ïÙî§z-OTHERbin2FGL J0955.0-3949CRTS J095527.8-394752?ÊÅ¢‹t'?̓ÙnÏI1?éN¿W]"à?̓ÙnÏI1?Ƒ"'÷?¾C¾6¥?ê[› B@?¾C¾6¥?â™âL?¶9zixu¥?ÛÉÌÌ:Åh?¶9zixu¥?àfÌÓ,ã8?²ÆÄÍs›?ß2fY¦9?²ÆÄÍs›?'x³Â{?ŽTIŏÑ?ïoô:‹'w?ŽTIŏÑ?"–G¿,1T?–¿Hñ.­?ïcMÂ"U?–¿Hñ.­?¿¹!]¹?®`Bg±ÿ'?ìÛÜ4HÝ?®`Bg±ÿ'?¥	^,îæ÷?bI…¶áõ?î¯jLŽp?bI…¶áõMIXED4FGL J0955.7+6940¿ïò²,LÃ@DH¼ƒ©mLÀ9EMÐÀ<_¶Q`Dä@‡•;;~@[­}|,¡?¨Ù#ƒy?®ø¤
]X@ç*ÙÈ]Ò?ü֘UKáÖ?ïÿ ~æ¿à+RÿTÿ¿á¶Gº©´š¿äß=¾.¿ã©<"?¾¿ç«S€Z®LOTHERsbg3FGL J0955.4+6940M 82?ïö#†©
;?H̟P%°¾?S¸òïÞ	4?H̟P%°¾?ï>גM ?¡ÒÉþµ~?˜<åŽâ	?¡ÒÉþµ~?ï'z•a?z?‰­zá˜læ?‹aZ¸Þ-r?‰­zá˜læ?ëî'Ç×ß>?©+Çþ¸?ÀE¸à ƒ?©+Çþ¸?ïÓ‡YÑ?p)Q¼^?vp<`Õï?p)Q¼^?ëWþ±úl?Ëüî'»[? …8P?Ëüî'»[?ï1Ø©"¦?"Û–'ý§?™ÄêÒ²š?"Û–'ý§?â
‡áhîµ?Àt²©Ð?Ûêð=."—?Àt²©ÐAGN4FGL J1008.1-5706c?êAhX Å¿ï<Úa
À8¥1G ¨'À:,Þ¨@¿¿>™Ä@>	»j¤º?ľ>ÿðÈ?ÀÀáÜÿIø?ü1¸ðiŠ?ûëøŒR?í'ÜEæ"¿ã°¡óÛ/¿åº &5¿éÜo6ï€V¿ã{ÕctCŸ¿îës`OTHERunk3FGL J1008.6-57061RXS J100718.2-570335?æLÂtjqI?ЩG^ZË ?Óf{+n?ЩG^ZË ?댰ãTL?•_vÚF?ÁÍ<sήÏ?•_vÚF?áGì¾.ÏK?»Ÿ™
Æ)?Ýp&ƒ¢ai?»Ÿ™
Æ)?êßKï0"µ?©`‡øY?ĂÐC=±*?©`‡øY?á¼^Cñá?Î$"¨hêO?܇Cx=Æ?Î$"¨hêO?Þü¶(Æs?Ôµz¬¶€?àð$ëœÇ?Ôµz¬¶€?෽ɤ¤:?Áÿҙщ?ސ"l¶·?Áÿҙщ?Ê÷µP-ë?¸ßíä:ã?éB¹ëô…?¸ßíä:ã8MIXED4FGL J1011.1-4420?Ê7£^®%@#b'è},|À;2*߈'À<‰3úÙO'@ "«#Ú¦?ÿdž!Ðý?Î['ãG¯?¥ñïñêém?Ý'½†,@¯»ù9¿â˜éÛÑLŽ¿ìez]"/Í¿à¶@º°@¿áñ–`)5ƒ¿š¢ža:¾©¿æÜ¿· ìOTHERunk1RXS J101130.7-442241?ïýÓҜçÏ?%ÜC©S?1am(…ƒÛ?%ÜC©S?ïèY"[µ?u3<æ¸Í¼?g¦Ý­ [T?u3<æ¸Í¼?ïók¥žX?[–½'æUÄ?Y(´|cpÅ?[–½'æUÄ?ïþX_…P?6snE?*z ‰An?6snE?ïýóBNÑl?(ÀÁš[öY?0eï;Ã?Ò?(ÀÁš[öY?ïK-"5?£*ï>wº?–šM¢ù°?£*ï>wº?ïöÌ:*É,?`¼	ËxÁ_?Rg‹½«w3?`¼	ËxÁ_?ïô ÊT;?R)àŽÌ':?WоÃMˆÑ?R)àŽÌ':AGN4FGL J1018.9-5856¿¤¶\"‰²¿úõ<WŸ#FÀ6*OÁß3À9­HJ­@øhÑz±w@rÇZˆ?•0£¥XŒ?Î_
¼òd6@6]3]$žE@/È´²¿ÊŸiKs¿àm	]¡Æº¿åyöÁgéÉ¿èàÓ¿Û¿í#>=ÓJ?¿ènq—òÐmOTHERHMB3FGL J1018.9-58561FGL J1018.6-5856?€bÚØ®:?"Ó›ÿíŽù?ï¾t"sâG?"Ó›ÿíŽù?¨D1±×(?¤c쟷&.?î{¼æiš½?¤c쟷&.?Ç©qt?¯†	bâõÄ?ê¾#¢Ø™?¯†	bâõÄ≯,Ì;O>Òròâ‹M?ïÿøÑÁø>Òròâ‹M?zp*wßGì?šÂ‹r'Ù1?ïË«
À?šÂ‹r'Ù1?{ߧpš?Ñl èow?ïÈAøàü?Ñl èow?°"™PO6?¢w;ÍjêJ?íïlÖ(Qi?¢w;ÍjêJ=ø"ë f!>#*ëSùšÚ?ð>#*ëSùšÚPSR4FGL J1023.3-5747e?ºÐjê_Ê¿ÚDUšfH3À7×xFÜ]À9›mjW@#_Jé2^@v¹<Íé?¶éπËf¿j&¶Ý?¾50¼ê¾@"Ǥſí(@éÈ?ïY¯¾ôòÜ¿ë[¨«¿ânŸð˯–¿ã»>U¦¿ÛþĖe×OTHERSFR3FGL J1023.1-5745Westerlund 2?ß:€a˾?Ôî%W?àb¿Ï}!?Ôî%W?ïM˜2š?¬sXüÁ=??–\ÞætÍ?¬sXüÁ=??á¡òŞŸ?¶k	2͕q?ܼtÂÁþ?¶k	2͕q?î"z͕cn?žØÓæþn‰?¦ÈS&©É#?žØÓæþn‰?äób…±/b?Ñ|®6‰©â?Ö:ô¡;?Ñ|®6‰©â?í6¤d×M¸?ƋHü{Ä¥?¶JÜ×û·Ã?ƋHü{Ä¥?æ¡bvþË3?ºËVž$÷9?Ò½;iš?ºËVž$÷9?ç ·»'=?ōxV±?оÄˆÛ†?ōxV±MIXED4FGL J1023.7+0038?{Z1ÀQ@Fä'úòÀ8Dœ¤æÔ¶À;ýÖ.u@ÿªó3=ð@Üb¼ºh?¡žÞÁ°¨Ä?Ç.95×@"2¹o!öË@½€šFM?·Y /_éõ¿ßa}H€!¿æ†_€>:¿èÅB>éË¿ì3ŒŸ`-¿ã'?´‰	OTHERLMB2FGL J1023.6+0040PSR J1023+0038?îüdʖ"?´‰1Ÿ? ?ɱžÏã?´‰1Ÿ?ïÝ7…C¨?€ZêA/ÕÆ?qd=z]‹ñ?€ZêA/ÕÆ?ìÆgs_PÑ?ªE#`,e?¹ÌÄeyx?ªE#`,e?ïöèê:ú?K*öìG+i?R.,füëy?K*öìG+i?íº€ô ²?¬t90úÔ?²+ø]µ—ñ?¬t90úÔ?ïYT.‰^?­šr0ÄÏð?"Õ}±—ÎO?­šr0ÄÏð?ìFêºëÆ?ªóÞZO?½Ï`ª(¡Ï?ªóÞZO?ïÀë
X?r'ÚZg÷(?Šyw"€·?r'ÚZg÷(AGN4FGL J1024.5-5329?è¸j÷^Š"@
çDñ¢À;1#³co;À<']9—@"?Öê‡ô?÷‡åÂg=?Ö=…³:?ÞAãd¾Æz@	0)®O3D@™zu<¿ïÿþøþ"¿Ê0™Ã?ïÿTßUe¿Á¡;#—Š¿ÒUÖ¿á±÷(ÀéjOTHERunk1RXS J102441.6-533141?ïöWÂ/\?R(¥%iø?SQÂ9¨Ç¥?R(¥%iø?ﴁñvF?'ÝèV¹U?'߃¨R"[?'ÝèV¹U?ïQ¨½¯†?ûQ…ÞÅ«?•Êèey;?ûQ…ÞÅ«?ïË5ÄÂs?hjÑûJè?zeÞ±ªs?hjÑûJè?ïõG'}Û?TÈ9Ð;X?UpÝƽì?TÈ9Ð;X?ínMηU?ÀPôˆ?´½'ÔÖ?ÀPôˆ?ïlsD´ÿ•?ü6Q2¾?'q—lÏ©O?ü6Q2¾?ïF´'m	÷?Žœ"âo?—){†+?Žœ"âoAGN4FGL J1024.5-4543?ÄÃ|äN–@#Àd©ÍÄÀ:´úŽ¦÷À<qZ»7y@ êÈÓmû±?þ"ä0—?Ä0³|Õ9?ªZÝ#å•ú?èaþÂé<@_£Ùäbk?ïéè »6w¿àN¦@Æç€Ç¯;¿Ô]´;0'ª¿Ñ¢5Ÿt$¿ãµ\"•¬$OTHERunk3FGL J1024.4-45451RXS J102430.1-454401?ïÔ{F¿¤h?²‡RÝ,?uÂ\"W?²‡RÝ,?ïâ
Ùo>ô?vêfê¼j?mõ&€Bë˜?vêfê¼j?ïóaŒ•'¼?Y‡ž(L_â?Y<æˆGõ?Y‡ž(L_â?ïò#‡TÙ²?@ÙÊ&‡î?[¸ñdZ?@ÙÊ&‡î?ïü>œjPÎ?8"ÓÔ†?>»
™?8"ÓÔ†?ï,æ)·€Ø?¤äY|
L?šc:Àxß?¤äY|
L?ïóŠñW"?e—fãµ®º?XêPÙób?e—fãµ®º?ï¾géÀšÝ?n"Qµ ?€f›ßêÃ?n"Qµ AGN4FGL J1029.3-6657?éÈå'tÀFr*rÀ:…úcÞ̪À;ñ讪¢Ö@ŽöÑX!Õ@WWÂHå?Æn=à¶8·?šOãÃ?Ø-™–>›F@Ï#¾Ì?ï
–V:‰¿è¸…íë*†¿êŽ
>¬ãù¿Ý¬ºÞ¿¿ã›â´•žb¿åPT "žXOTHERunkPMN J1029-6656?ïþ"_‡?#Do\ ?/¿¤gð@?#Do\ ?ïñ~ƒ["?gRÖLäpi?]ùvÒXù?gRÖLäpi?ïîqÀ6¼U?fî»>ÄÞ¯?aŽ?´¦m?fî»>ÄÞ¯?ïý¤2FE¬?MÁõö?2Þnõ—dÛ?MÁõö?ïúÌã%²J?FÂñv	O•?DÌtH÷F?FÂñv	O•?ïµÞN'Ö?–öù۞ƒ?'ˆx©óА?–öù۞ƒ?ï×2È:?~ëÚÒq˜ô?tfû͙c?~ëÚÒq˜ô?ïów›íܽ?J¢Þ¼–*?YÈGÆ[?J¢Þ¼–*AGN4FGL J1034.7-4645¿î3U—k±@#Û,B»fÀ:ïùZÊPòÀ<cÐÜ&$@"pçɨ@'}ô!¥?˵Ï_‹+? ¿5#g'?Ԇ$¼øÄL@¹9õš }¿¿'£ê¿ê±(+˜4¿Î§!—¿æ]gÿî<¿ÊçFu°0_¿æÎbß\\OTHERunk1RXS J103438.7-464412?ïþ6œ&ð?%ç»ÙUz?.̙Alk?%ç»ÙUz?ïé,þ!Ý?tÿâ4{O\?fÓÑ-³?tÿâ4{O\?ïòuá-¬á?e'Mì¹?[>Ú?e'Mì¹?ïþk¯a¾?¥KÛüwÔ?/9D00?¥KÛüwÔ?ïþšq}=?%'»Ý;Õ?.]$J€?%'»Ý;Õ?ïTr"Elœ?¢YHø"?•q­•šžŒ?¢YHø"?ïñýÏ+ÕO?p	òºJ¨Á?\ai"O?p	òºJ¨Á?ïöªª²,?GP¢£/r?R«Ì4i¾?GP¢£/rAGN4FGL J1045.1-5940?"߲úàÿ¿ãüpÿFœÀ6høj	‰À9êƍîj¬@î«Ä¿b@©²=ÕM¥?'Šg!¢<*?¼Ø;•ØCù@'Ú^±¬@¿+½óëö?ï(Åñç9¿×q10–v¿ãì2žðÔ¿äTµÏZEÇ¿è°&äpX¿ä¹Ùk€,OTHERBIN3FGL J1045.1-5941Eta Carinae?å¼åÒ¾d?Ö©"' ‰?Ԇ4Zƒ6ß?Ö©"' ‰?°IcWÈ{Ë?©¸,{aŠ?íöӔù2?©¸,{aŠ?å	zÞԝb?µª¨e׸?Õí
BVÅ<?µª¨e׸?­*ôȯÕÈ?Ÿ˜D¸0?î-P³KÇT?Ÿ˜D¸0?Nj"¯ð?Ì¢3¯bŒE?ê>ܔ?Ì¢3¯bŒE?€8ÑÅ'??‡®¥dfÿ?&Û??‡®¥dfÿ?è!»»ú¹ç?´‰ïÖDÎD?Ïyb?´‰ïÖDÎD?B,(U	¼?=ˆ£ÇU?ïûµa?=ˆ£ÇUMIXED4FGL J1045.7-6414?çIiÞôuÀ'C{À9Ϻ˜í¢/À;¼áG®{@báK´ß@"õ?²w?Ã>ZÕÈI?Æl–\ò@\,CTéf@裉1—}¿ïþ¢˜›Ã?ïúiˆYÖ5¿ã÷M©Öþ¿áJ·~†îœ¿ìSá~Š ¿èú˾!OTHERunk3FGL J1045.3-64141RXS J104537.2-641438?ïꯌÜ-#?n7®ç
p?ePrëyE?n7®ç
p?ïÆáúJM?HwÞHù+?|úî=1z?HwÞHù+?îø­Q÷x?•»£)û? u*ÝìŠ?•»£)û?ï‰i Ù²?qû* ñ'[?¥ºž¨Ë[?qû* ñ'[?í¨˜˜›J?·œ_Qt;ç?·*»<òóª?·œ_Qt;ç?î\¶µ^F?µ|xuõŠ?ª>d'òMŸ?µ|xuõŠ?éøT)øÌÛ?¶¿¹–ü?ȯX̔?¶¿¹–ü?ìÊmÉ©y-?§^î¸<ú?¹¬'²´6˜?§^î¸<úAGN4FGL J1051.6+3253¿Á9íü66@OÃ˼+"ÙÀ;'?Ï"èÀ<êՌŽï@û´ò»sß?ÿ†YJôðØ?×ǘšëÿ?©	%B¯¨?ѱÁ"õxh@BÜÔ+æ¹?ãxo'Á¿ïÿôw5Áƒ?ïýއà3²¿×E;ÿ	µá¿Ô—Ø"¿ïÿe`õäOTHERsbgNGC 3424?ïÿFD†S?*g'`B?7v!Ý ?*g'`B?ïø(Z½ë?QFàÞw?O^•Öœt°?QFàÞw?ïòt/ìp›?gákÌ¡¾?[ B›ª?gákÌ¡¾?ïþîÍӇý?£M¢Û¯?!&XlÌ?£M¢Û¯?ïÿ¾fÔ>ý\&táÕ<?~=ˆ7ª>ý\&táÕ<?ïÞۓAÄN?s|,g8?p'6?q?s|,g8?ïõ·C<""?gªÔ¨Ó:?T'yvx×&?gªÔ¨Ó:?ïþ¦¼Aå(? Bëf…ºþ?%"7Þ»ã³? Bëf…ºþAGN4FGL J1059.5-6021?ì#%Êûøp¿Ü¾Ò
SÀ9³9ä'À:š>—ëC°@lTi¹­
@ªÂT£Æ?ÊäÑ{]C}?Ï$_ZÙjj@>ä\5Šü@2\sž]?ɖƕüA?$Ç/¿âa4x­'¿æ¥'ßæÚë¿ïÿýç!é?ïÿ·pD5ºOTHERsppSNR G289.7-00.3?éñ:ç#?Çä€ï9ðM?È;ìcs ?Çä€ï9ðM?íBÅA4 ?¶:óž'=†?µéÕõíï?¶:óž'=†?ç^&"¸?²£OÜffÊ?ÑC²öüø?²£OÜffÊ?퀉u½¤ï?œnE½U^Í?³û´Q¤å?œnE½U^Í?׀Ûö>é?ϜÚ-â[?ä?'àöŒ?ϜÚ-â[?Ú½"öÈ?ÒeT¯§?â¡="ðÀ?ÒeT¯§?Ø9°˜0/?º×ÏV·>?ããt'³çè?º×ÏV·>?Öu°¦{R?½ƒ™ä(oF?äÅ'¬Â@W?½ƒ™ä(oFMIXED4FGL J1114.2+0638?Öiªþñ¸@M'ËÿGs\À;¾vÌ7«À<Ø'QT†@"_©mø,?ÄWoRž2†?åÄáçDò?ïûo! ä'?þ8¸É	É­?ø2¥4M¿éç÷Ë~4¿ïÿߞ¶Žó?ïÿ.´Hq‰¿äÑq5Í?ʌ3)£'¿ìYƒ)Ì@OTHERgalIC 678?ï÷@¶13?j{?…Ö?QÅPÊX?j{?…Ö?ï寻U<Y?‹íÈöE?jPD£äoX?‹íÈöE?ï;=^Ág¥?Ž‡‡²â!?˜˜T,úuW?Ž‡‡²â!?ïâ1·?c^Ÿûaûh?mÎúd°Ç?c^Ÿûaûh?ïá©%'×µ?q¡ÀE´ û?nVÛâúa?q¡ÀE´ û?ï¯QÜ
)?š—)	¶"–?"?«Ì)¹?š—)	¶"–?ï6M0/b?'"$]›?™6__!}È?'"$]›?ïãRe±e?sɊ¹\  ?l­š€gû?sɊ¹\  AGN4FGL J1128.2+5831¿éè›
`Î@K¶-VÀ;b°+¬VÀ<ёúhçJ@Ó£åLöS@îÛŽ,?Ð{uâZR²?¼oa^®?íÝe k/y@Öm¹kñì¿ãPxˆ§ÙοévýÃÝé¿ßäY±L¿âmf4è?¿ëўJÙB?Í×͜U‹£OTHERsbgArp 299?ïû¦Ã½sW?7㥤ìt?Adð°–lÄ?7㥤ìt?ïö¤*Ru)?R¨T0"™r?R·«°Kýy?R¨T0"™r?ïȹŽâ<?x7"Û*Í?{£8ß±Š3?x7"Û*Í?ïó4ãêÿ?B›<#×g?Y–7Á«†?B›<#×g?ïûÈë8?.?8a¦³L"?@ÜSä`	÷?8a¦³L"?ïڊ~YÞT?s;'æeî?rºÀá1ô?s;'æeî?ïÄ "›¿?ƒ=÷p³?}¯µ³€Hƒ?ƒ=÷p³?ï°È›ºd?sôjù…¬?ƒÍØ¢c?sôjù…¬AGN4FGL J1151.4-6248?劸'ñ~¿çz¾ï>'À9!JÕh-À:À´†"éß@'éçÆ²@ê²ái<?ÂøScTc/?±¨Ã
†P?õ§ðª!§@²™Å¹?Õ-GáÀú²¿ßø€‹*Á¿ê¾9÷r'Å¿ä"ô¿7G¿æV‰äð°¿ëaÚ`3F~OTHERsppSNR G296.1-00.5?ïÅ&{Ðìþ?ÇþBÐÞú?}lÂ%Gð×?ÇþBÐÞú?ï˜Õõü'-?'eæä¦f?‰Ê's!¾?'eæä¦f?í1¿bS?§³±äÇÉ?¶w¢§Cc?§³±äÇÉ?ï]'(sÙ?zÛ/Ëӈ?"MÚåz~Ý?zÛ/Ëӈ?íë÷ºQ±?±å¨gõª?° G+å@t?±å¨gõª?í&_ÇÄX?ÀyL¡??¶ÏŒÿœÄ?ÀyL¡??ë1]o
¾?±¯¤â'ÉÛ?Ã:ŠCÕÅ?±¯¤â'ÉÛ?éJš¶'¼?´áʨÛ?ÊՕ%õÀ?´áʨÛAGN4FGL J1152.6-6207?å÷u #È¿›N(¾ rÍÀ9ÕrQV3éÀ;€ö4¥#@åQ(À@%iF·G?Ô: $x/g?ä{àK.Ò@Rµ¼åÎü@Á'kՑ¿é%÷@=ݱ?®T˜€uv¿æbÀi'¿ë›[Õì¿êC,oʓ7¿ïÿü¥¬¨OTHERsppSNR G296.1-00.5?è§Qñ—æ?Çòi§Âú?Ï©b¸9 h?Çòi§Âú?átߕHÉj?˨ßÞwo?Ý@Õnm,?˨ßÞwo?è½4ë]öD?°\,Øys÷?Í,Rˆ&ï?°\,Øys÷?èëüР–ä?«'°Ž?ÌP½}¤q?«'°Ž?Ó|ød¼Si?Çßtu®éô?æAƒÍ¡ÖK?Çßtu®éô?ª¤œÐ,i?µB"ºú¡Î?îU¶3
÷Þ?µB"ºú¡Î?Јm•bZò?³+î¼eëO?ç»É5N҇?³+î¼eëO?º"¦Ò?ª.ʅÚ%ú?ì­k=e¼?ª.ʅÚ%ú	MIXED4FGL J1155.2-6259?ÑçÅb0‡î¿éè:ÛÀ9'6TOãmÀ:—yóáäŒ@"éµæ¬G@¸5u-?òƤ^ïy ¿îL?á&£7¨ú@Öð<=ž?ß¾Y¢2ÅO?âKÕážk¿ç˜}Ú÷1û¿æ/Y‰ß¿é«^½ûx²¿æÓ¾ŽE¨OTHERsppSNR G296.7-00.9?ìÇ╝?ǾI±ú¹o?¹Ç(ëS!?ǾI±ú¹o?ï Ñ?^uè?«ÜÑÔRåò?›åØ	Øþ?«ÜÑÔRåò?èþÿ÷"í*?²iX¡;Uj?Ì!°KY?²iX¡;Uj?ï7É>4"?‹?òî¦d¤?™ØEØ¥"?‹?òî¦d¤?çë*î– =?̯ÙŸps?Ð)ª"Ó¿…?̯ÙŸps?ì˜EÏ šG?ÈNêÚåû?»=тû-Ä?ÈNêÚåû?èâùo[ò?²:
N©?Ìw"B7?²:
N©?èùӐ,ÕÃ?½±)1–iÓ?̱¿L¨ò?½±)1–iÓAGN4FGL J1155.6-6245c?т88º¿â'óøŠÀ¹À9+û¤P¬ÁÀ:lE(þüË@Ö*%mwÓ@íÍÛÀ…—?ËJY™??Ñäg¾U:Å@‰óžÈ­ƒ?ö'ÞÉN"¿ç€E4½vî?熁žü?ŠºDΪâ0¿èÒ­N ¿ëfÖ-¿ïÿõEq#OTHERsppSNR G296.8-00.3?Ô%Pœz ?І®)Ú«?åôíW±Â°?І®)Ú«?Ï ÞeBˆ?ÇaòQO?è7Èf¿/^?ÇaòQO?áaÖIžQ?µi åǨG?Ý<SÿlÃ^?µi åǨG?ԁœ!ß"æ?³H…?å¿1ïn?³H…?Ém‰45?ÆOúSá€?éº$²ò ?ÆOúSá€?"F	ó €|?Ÿ¥½C‹Ô?ï]Ï°pºl?Ÿ¥½C‹Ô?Á–öYÁšó?«ÐÆHҖ`?ëšBi™C?«ÐÆHҖ`?ˆbG•Ð=?{Øyü	ï?ïžwú¸mo?{Øyü	ï9MIXED4FGL J1158.3-6232?Ÿ±'gSÔÇ¿ÒØ>e@v"À9)Þ®v pÀ:½¨ö-ï'@ XQÀ'ô@Jh˜q?Çm™I'›?Äug5CXÅ@nÜV­Œ@»{–¤G?î"ßÄK¿å´—1š­¿æÂB/Oy¿çñ§w¨®¿ë­ÌŸJ¿éë֙Õ)OTHERsppSNR G296.8-00.3?ï±L	)/µ?‹øø­Xñ¼?ƒ¬ý»3r ?‹øø­Xñ¼?ï`	¨ÓÑ×?ÕOòÐ?"þÊê­/?ÕOòÐ?ìScÎAÓ?«1ì²×io?½dáñg-?«1ì²×io?îø–8ÞeH?ˆˆÂ'Ô[÷? vœt­`}?ˆˆÂ'Ô[÷?íìFVÈÛô?±ÊÌe‰ô?°ÍHRd?±ÊÌe‰ô?ìR!9´?Å
G•"¥Û?½n÷?Î2d?Å
G•"¥Û?é	§$¢?±'ëdèaÿ?ËïÙc«my?±'ëdèaÿ?æ|ß=""?º1Ñcñ?ÓA"üöÙ?º1ÑcñAGN4FGL J1159.3-6122?ÂGÉ|O½?ëýH•›À9Öƒ.ô	À;šCㄟ@Jö‰‰¬@¼*`%څ?Ì)ž‰îUß?ÉŌ§Ük@_î¥d¨÷@dHÔÛ.?æüóÁ-\Z¿Ø¶ßz¤`ó¿á-ÆwH5ú¿æQ6É>£¿î	¡Ñv¿ïþÙú²¹%OTHERunk1RXS J115843.7-611934?î×GÝ©?£¨ÿyX˜?¢Ž~µÓç?£¨ÿyX˜?ï7ÅOf*è?™Îbû­õ?™V:¢ò?™Îbû­õ?ì°é»…?¥=ÝÓ|·?ºÀ·b#Ù?¥=ÝÓ|·?îÏS*?"x¡µ?£
΁«?"x¡µ?æ|ΙøÜm?Ɠ	Ò¼¥ã?ÓbÌG'?Ɠ	Ò¼¥ã?ê™OUía1?ÅCwV¬=?Ś¨J{=?ÅCwV¬=?ãk`ñåW?¸£;¸¸¤¿?Ù)>Ä5Q?¸£;¸¸¤¿?æ¾ð'ÖÖÞ?²
 q=ôœ?҂úRRC?²
 q=ôœAGN4FGL J1208.1-5149?åog¼|È~@$ô‡Tów\À;t2À<kAHŸ¬@ oÔn+ן@.Ʊ?Êœ§@ W?¬éᅖ'c?äõ"FK=ì@9ʎÙø?ïÿ¢­>'¿é̱‰zg¥¿à˜Øÿ`ö¿ÚJS`OK¿éÃsݝT?ÌtÀÇ/ÿÍOTHERsppSNR G295.5+09.7?ïíÔùäTu?—1äü÷?b+.ªâ?—1äü÷?ï滘ûm?uò(æÐò]?i÷D@ˆó?uò(æÐò]?ïä>6_Q?qf½.`Cï?kÁüúFO?qf½.`Cï?ïørqPi?4|£Y€ã·?N6:2+¥c?4|£Y€ã·?ïûрqÄ?=H'|¦jY?@¹ÿ¯Ð‡½?=H'|¦jY?ï:ožãb?¥"Æz5«?˜²tÉÑ?¥"Æz5«?ïÕ›Á'?{û'¬ËZž?u@2Ødý?{û'¬ËZž?ïÞã³EÇ?^½¨¬Ûåt?pŽ&sÝ{?^½¨¬ÛåtAGN4FGL J1208.5-5243e?ßyðŸS²@#0FÜ]dÀ9#V›‡À;ŸâV¡ÍE@ eSµø ?þÙû‰xº?«¬=
LŠ?"XÖʖU†?Üyb—yÚ?øˆmÅ*l?ïõ΃†1Þ?ïŠIˆà¿á÷=^ZS^¿Ö&Å#
F¿àêâ«¿ØÙ	Üwº¢OTHERSNR3FGL J1209.1-5224SNR G296.5+10.0?ï÷dN6D?G—ƒtl'z?Q7Û¢ÌGë?G—ƒtl'z?ï—	"'OÀ?"iÀX¸7p?Š=·N>%?"iÀX¸7p?ï‡MÊ
TÒ?‹ÊYÁ|?Ž,u˓z?‹ÊYÁ|?îÔöq-a/?'èãŸEV×?¢°˜í)í?'èãŸEV×?ïÜaFZÇ?g‡hR›v?qÏ\åÚH	?g‡hR›v?íîñAêö?·äè¢…?°ˆwg:'Ð?·äè¢…?ïuÍ<nä?Žãí7ë?'FXyʹ{?Žãí7ë?ì"`c†ÑÛ?®øÖφſ?»\üãÉq+?®øÖφſAGN4FGL J1213.3-6240e¿ï¹@󇙿À=çՒïÀ7@)íÀ:,…dž@™bRZ•Î@¨]Ywj›?¡‹:ÜúA?µXè_¶…@lâ¬2#@z$b_ñ'¿Å¥'Abv¿ÕàQ<¿ãyâyÝ;°¿äv†¤ÊOD¿ç#ĀM`¿ãhë¡y6ùOTHERsnr3FGL J1214.0-6236SNR G298.6-00.0?ٌN^Kª?Ò͞­ ?ã9ñXÐÚ+?Ò͞­ ?Òµª)?ÆÖ Ëf?æ¥*ûðë?ÆÖ Ëf?ã)rk=¡Ý?¶6Ðg.`?Ù­)"¼E?¶6Ðg.`?ØËåÚm|ä?µ÷¦°§~ê?ãš
ÉAŽ?µ÷¦°§~ê?ÓևÇÆ?ÏñÃ,Ñ´?æ{ö¼?ÏñÃ,Ñ´?–ÀºšÆ?Ÿˆ¸VAÊ?ïOùæq ?Ÿˆ¸VAÊ?åÜ!?¯‡0?¹ºDö.d?ÔG½€ ñŸ?¹ºDö.d?—üäŒvG?ŒU]JKJ?ï@ÜZ¾?ŒU]JKJMIXED4FGL J1256.1-5652¿Ù‰hôá@ùú}	@À9Ð)é•öÀ;¤uÓÁ³"@/=;tË.@"|tÅ¥?Æ-+²5qÒ?àD@÷–û@{xÎø?ø=ìl¥DÉ?ïúÂT£Æ¿Ú%›eK´3¿é1¦€²Âà¿ëxöLÖó¿åŠºÙ…Aô¿ïèP¶Ñ¸ÅOTHERunk3FGL J1256.1-57031RXS J125554.2-564945?ïD³´U3?žÁUX?—i‰zuc›?žÁUX?ßgwÈä_æ?ÌêœòШ¶?àLDÐ
?ÌêœòШ¶?쳟¶'ø1?¢üñZZEo?ºcKè>v?¢üñZZEo?æ²9ƒB?®Ð=úÊR?қÎùç|?®Ð=úÊR?çÎk\ç®ó?ÈʬRÐÝ?Ðc)F0¢?ÈʬRÐÝ?¤#ÔSd½?¯êlœ•µ?î½Â¾ßä?¯êlœ•µ?ä29tڌB?¶GfR?כJç|?¶GfR?¼'ÁûbŒg?©I/¤×g?ì{À"®s?©I/¤×gMIXED4FGL J1302.9-6349¿ëzð5¹©¿ï"ÃÀ8Ôðý-½¨À:Rj¢Ž5@;ó HŸ×@#v"Á›@?µåš¡+‰¿µý 1
i@\[›1IN@î1·?ïÜ<a/Dç¿êUÈßWhó¿íÉÂVQEm¿àÚ!2Æ¿ædÆ®0*?¸iE~d^úOTHERHMBPSR B1259-63?îlroÞØ?·Øí"Ÿë'?©8ßø&+‰?·Øí"Ÿë'?ïéBÞÄ=?y¹Ì¡M'?f½!g½;?y¹Ì¡M'?êõ£L9®;?°ªB{ìÊ?Ä)rÏG?°ªB{ìÊ?ïÿ±yMŽ>÷S†òD*?ºò
µ">÷S†òD*?ïe¼0¯?¦,΁ä¹?œ]ƒR€7?¦,΁ä¹?ïK!S·¸?¨ßó`®mF?–›Õ€q÷¶?¨ßó`®mF?ì%ÚD&
?°·,$í?¾Ñ-ÞÏG•?°·,$í?ïý©BGçå?06µ‰Bù?2µïb'V<?06µ‰BùAGN4FGL J1303.0-6312e¿ìD>H¿ÖáU…m'«À8EñÓò[À:ҕˆ'á@"'|2iµ?ýÚ8
2ˆé?ªO"›Ø¿£e">=¨W?÷ˆ•âU?ûÈúDÕ'?ïh«…Th7¿Ø6rûé¿àÛ?÷fÔJ¿â…`\a)ç¿Üíaw¤Q¿ÃQu¾sÐOTHERPWN3FGL J1303.0-6312eHESS J1303-631?ﶻÁÎj?Eaº?'QÇC[?Eaº?îÕ«ːs?°ô¦³…€?¢¥NóFøÒ?°ô¦³…€?ë¬M®^¢£?«ò«iá×1?ÁNÉF…uu?«ò«iá×1?íYö>hÎÿ?¤ŠŒÌ±½à?µ0NqV?¤ŠŒÌ±½à?ï#ö™ÏÕ?™«Ÿ«x'?›,Õÿf?™«Ÿ«x'?ërˆk§v…?ɦšo=·?Â5ÞQb%î?ɦšo=·?ì°»Œ]›ç?¬}þ2 f<?ºz# Ä?¬}þ2 f<?ä£Õ\4֙?Á€¥ë¯L?Ö¸UG–RÎ?Á€¥ë¯LAGN4FGL J1305.4-4928¿ë€~ˆ ~@*«h'0ÆqÀ96s¾=½ÑÀ;üR$A@Ò@VÝ1t@êù>?­7›!Ùïu?«ì^Ó¶²?üuÞß)@¥^¿þÞ?¹j£Œâ|¿Ø¾U{1¤"¿å™ç'Z¸³¿á¾'¼ÞB@¿çpÖAj®u¿àâ~å¹-OTHERsbg3FGL J1305.4-4926NGC 4945?ïõ3f	þ?L—[Yd&?U™ÿL©4m?L—[Yd&?ï'Ûv€?ÁKk6¥q?~·v£WÖ?ÁKk6¥q?ï»ñWñƒ?ƒ0ùß`¢?ªÕá?ƒ0ùß`¢?ïŠJÖ+ßò?v£$4£,ä?mJ{ç;•?v£$4£,ä?ï¾™µ•›?vÇ¿ýƒk?€`"J…??vÇ¿ýƒk?îaC˜ÊÖl?¯€€Ãß¾A?©ëÆvÂ56?¯€€Ãß¾A?ï'9XH?–wDÄ¥íØ?›ßoÈ­?–wDÄ¥íØ?í†kûŒäç?¡m3oz("?³Ì $ÌK?¡m3oz("AGN4FGL J1305.5-6241¿ïz=]P	¥?Á9Û×À7Ù\M}À:\Ê4lW@xƒ
¼L@ãö<1ßv?­R°Å/J?¤§Q"¤q?öéëÜ\ŒÉ?ùÒ¼­ð¾š¿Øž½ûx±Ã¿Ú)²ÒÛ¿âþtàÀ˿㕮Þ]¿è¨Ÿ%ʔä¿áýiíÚcŽOTHERsnr3FGL J1305.7-6241Kes 17?䢌Mf÷A?ÑÈ]}oӉ?Öºçe2~?ÑÈ]}oӉ?íçÝón"?¶ƒ\'˜z?°Áf`¤^?¶ƒ\'˜z?ãÅ7_ÆB?¸Äý¸Ø?ÙØu'@s|?¸Äý¸Ø?ëV‰ÍlI?¯Š/˜Ïí?Â¥ÛÀÊNÝ?¯Š/˜Ïí?ϋôäÝ©ƒ?ЌH"ˆš?èÆȕŸ?ЌH"ˆš?拞	H†µ?Ñypû{òü?ÒèÃínò–?Ñypû{òü?äÌ÷¯Eõ¥?¼ñ™åÅá?Öf¡t¶?¼ñ™åÅá?Ø,Uðê?Â};Ì×+?ãéüU{‡‹?Â};Ì×+MIXED4FGL J1326.6-4729?×?««Y@-êy5v'À9C	A}À;å±^²<ÿ@Û¶ˆÜÌ@KÌå €©?´"=l@?àùíÌ÷"÷@'eØם
g@PôF¹?ïdC¬':׿ÔPá_ø¿Ô¦êk²¿äè+Íä¿î¯4¬¿ïÿÿ" 5•OTHERglc3FGL J1326.7-4727Omega Cen?CwÈðù(?@öÉjxá?ïû"	0?@öÉjxá?³îçÉ"T[?±Îþg©?í'#ðÄ?±Îþg©?™ÅL¶ù,?³\ۚ'_?ï1՚H7Ÿ?³\ۚ'_?~*åÝWÖ?q+†6ã?ïê5~ ?q+†6ã?RYue}u[?r@;Ӎt?ïöÓE";?r@;Ӎt?ŒÈàŽ]–Ø?'ÕB°u?ïŒÜ}«Å?'ÕB°u?‰o·ìíˆí?x. Etª?ïšA u…,?x. Etª?
²Ä¯³?

lÛÆ-F?ïÿ…‹'\?

lÛÆ-FPSR4FGL J1331.0+3032?ï¡5DZx@T+ü27‹À:ւè},|À<›µäRûP@ž&ÂaŽæ@ŸŒÝÉtS?Ç`ñ\y'´?ÅüÚ܄ü?ýšMÀg?ü´P^è×?æ)ÖÈÏK¿çñ¢ÚŠûq¿ç`Á`ÝæP¿ÚOó]ZN¿ì°-…C¡¿ïýM"ŽÇOTHERcss3FGL J1330.5+30233C 286?歷¶~¤?†å
¥õù?†\Òq…?†å
¥õù?î•
ö¸?¯Å©ú²/µ?¦¯'äIƒ?¯Å©ú²/µ?ïtÑçF~G?‡À!¾w¼¨?'eÃW¡?‡À!¾w¼¨?í@híC(¸?˜—)²ý­?µü¸—0"»?˜—)²ý­?킿,}Ú?°:£4ò«?³ê.³?°:£4ò«?èZ)Ü?ˬ}µ@×?ÍûŸÂ—X?ˬ}µ@×?îT»pÙÜÖ?¡_hþï?ª´Hó>¤?¡_hþï?áXZ¹×I?¸@m¸¨?ÝOJŒQmÂ?¸@m¸¨AGN4FGL J1343.8-6208?Ú߂íП?»õ|"š7À8ƒ%{º‹'À:E×z¥¹@[#¨üŽ@ö"|#g
?ÆGX™Ÿ"ð?½|_LØ@-wœïo?î~՟ž?î|äù¿ÒŒewS¿æBaP™¿çÉâ!GÎK¿ê	ÿ\–¿åì†;OTHERsppSNR G308.8-00.1?çŒú¨ôå?Ò1vÃ^l¥?Ðæ
¯ö6?Ò1vÃ^l¥?Ý©É'$«?ÐL2%ʝ{?á+7mª?ÐL2%ʝ{?Þ,ÏñZ0?»ŽW­L:?àé˜{Òè?»ŽW­L:?ÛÅéAÂî?¶¥ï¸;¦?â{߉?¶¥ï¸;¦?ÙÒ
ûÿ?Õºmá?ãùws€?Õºmá?®ùԖëuw?¼dWÇ«ên?îb¶ƒŠ9?¼dWÇ«ên?ݟõùÁÍj?Á—§·>›?á0K?Á—§·>›?š îá?b¦?‹ÌN\f§?ï.øˆèF{?‹ÌN\f§MIXED4FGL J1344.9-6228?×P~Vêj¿ÏnëE2åÀ8¹ŸœÞÀ:4܃ùõ$@è8<ÝV@‰ÔDRÉ?Å¢ÁvŽö?Ý[ÔýrÜì@ìý
y@,:Z™Ô?ãH¶‡æ鯿ٕ˜ƒ$"¿ÚMy£¨¼¿èˆôe˜
M¿î¦âÂØWE¿ï×ÁÝÛgðOTHERspp3FGL J1345.1-6224SNR G308.8-00.1?¡€•@ãWÐ?³¡Øìæ?îçö«ºÐÃ?³¡Øìæ?½Ì÷¦%?´s:Þ²¯?ì]†a;P?´s:Þ²¯?ÁX¤~FyX?ªôwÀ
É-?ë©Öànaª?ªôwÀ
É-?ÃÎ
Ã?©ÛSZ]?ë9yÌ}O??©ÛSZ]?«h<]â?Ê
u®¶j?îI|:/ž ?Ê
u®¶j?…T9ú2ò­?ˆB1Øß'?絛Ò|?ˆB1Øß'?—t翉›´?‰Ê,)@Ї?ïDXÁÚwÓ?‰Ê,)@Ї?iqØA˜yP?[Ñ<'^?ïæŽ'ܤ?[Ñ<'^PSR4FGL J1345.3-6253?Ú›4ƨ"¿äâÙÿePgÀ9L[[piÀ:¼2JÕç@^WÏâ@ª*sq?Ïý‰˜š–?Úò²Ú³?]@!móùa€@óI€Òx]¿ïñ7æ Zé?ï•dSN\¿á`ÊžUì¿ç{wÀ*ýÛ¿ïÿÿÊPË?ïÿК·¦ËOTHERsppSNR G309.2-00.6?Æ¿þ×¥²›?ÉÇô5q{î?êPJ"Y?ÉÇô5q{î?ãI+aF…º?Íî¸Ç~¦œ?Ùm©=rôŒ?Íî¸Ç~¦œ?áã§@Ú?·NlÍó8?Ü8±~ßüL?·NlÍó8?êëK¤²ì?®ç¥¢-ÀA?ÄRÑm4O­?®ç¥¢-ÀA?¾ót_<?È7´8ù"!?ì!'tü9?È7´8ù"!?«ØÁûj?´Ñxx/?îBsàwy‰?´Ñxx/?ÀnóŽé¤?ª€am»ìÁ?ëúäCE—?ª€am»ìÁ?Â~`øé5?³·OŸëçF?ë`çÁų?³·OŸëçFMIXED4FGL J1355.2-6420e¿Ô(é°T¾kÀ•;›·À9¶N¼üuÀ;w™÷j·@%tÁ¾¢h?öªî «†?¼wbâù4	?§¥C_¿òã?êyÔ½\@UaµQ°ø¿ïòl~®[È¿ïì "ÚÅ´?é•\¾Fø?ïýaw]¿ÙÆ|¼A%¿À]GóÐGOTHERPWN3FGL J1356.6-6428HESS J1356-645?ïô·Ö½–?š3ÓY=dä?VS8ýó™?š3ÓY=dä?ïã½EµÉ?}ªO†:k0?lBº6]F?}ªO†:k0? XSî?‰é¡f9f?ŠÔ7ߜ0˜?‰é¡f9f?ïèË"1?bã¹Æ]Ä?g4ÞkR¼?bã¹Æ]Ä?ïóªNMÁ?U½ÌˆÀ­?X«óî
?U½ÌˆÀ­?ïe¢
£¿Z?¦VîŒx?"K¾®÷°Ã?¦VîŒx?ï
"!Â?—šî¨?œœ^M›ÇÐ?—šî¨?ïÃp«l]?€pªmÂrK?~Gª^nèn?€pªmÂrKAGN4FGL J1357.3+3730?•ü}ÉÂFÛ@R+µ^ñýßÀ;ÂD—Å¡À=ÅÉ£L¡@ k°'­¼ç?û'²z;/?ݲ~ñ"?ÔP`j£âÉ?ö‰ì˜D/?ú(¥é34á?åŊƒ| ã¿í]ï3ÿáÍ¿È`—D€¿áY+€Á¿Ôãr@9V
¿ïþëbº	|OTHERgalNGC 5380?ïòH£C!Ï?R~(ɨ£?[n¹Á4AÁ?R~(ɨ£?ïÒ?Ê4/÷?ƒ§jJË"!?vàÊk$?ƒ§jJË"!?ï˜TÞ\Ià?ƒ§"ÊoÇY?‰êÈhí‡á?ƒ§"ÊoÇY?ï‰8Þ÷O`?t˜X½•?±ÈE›Ä?t˜X½•?ïçß¿1v?i¼Õb	?h A
Û©ö?i¼Õb	?ï1¨'"!b?¥JÏÅÆ5h?™ÊíÖ[¬?¥JÏÅÆ5h?ï^DHÚ9r?Ø8 6j?"7vãÆ?Ø8 6j?í½˜7Ï?£'ž—"¹?²+<Z(‰?£'ž—"¹AGN4FGL J1358.2-6210¿í¾ùKA--¿ÓwÂäì~CÀ8SÒkr>âÀ:WoÈ@ã'4pJ@[#<E*¬?»5€•f¯?Ѭ‰á?Ër@íwàmò?û'ºz9×è?êœâß]É	¿ÛÖqüœž1¿ãŸÕÞCl¼¿è±·Ÿ¿ì踻Ð`¿ïýáÃÔ×OTHERsppSNR G310.6-00.3?ÔC&ƒÐ@?ÒÜ'LŽèª?åÞlò>à?ÒÜ'LŽèª?ÂQO—±¦Å?¹'È20$?ëk¬–O?¹'È20$?ѧ­g<?´²²
?ç,){úLb?´²²
?ÅÓ½üÕ(?¨'Y"Í°U?ê‹¿Àʶ?¨'Y"Í°U?">KÍ?ÁRÅ#$<?ïß)Ã?ÁRÅ#$<?‰D>e™Ì?1"0ê}?ï›îï(	?1"0ê}?•R~~ÀbL?ŠBlaÃÒ?ïUlÓ.?ŠBlaÃÒ?ožTáN$(?`Ïuéz#?ïàa«&ðì?`Ïuéz#PSR4FGL J1404.4-6159¿í·jŒ)³G¿Ôq1Ûð+LÀ8!‹P*º¿À9µ+†–‡–@–#BzN@í§m—³?Ä9å>ˆ¦Ø?Ø+G¬fû¸@…ÂL@J?ÿBe"C¡À¿à-Ný¿?¸óºLl•*¿åA1ÃÇj¿ì4œŠâ¿ï«±äéú¿ïäa¾áҘOTHERsppSNR G311.5-00.3?×ø­¤
?Ôéµq¢•Ó?äö©-úÿ?Ôéµq¢•Ó?¾zµÏksÓ?µ}ƒ•·'ñ?ì0©F'†?µ}ƒ•·'ñ?Óú™´F™?·
pýXa?æ³%ܳu?·
pýXa?¼ˆ:K«O$?¤G1½è?ìnø¶Š–?¤G1½è?ÕñŽººÈá?Øm¤`ûv?å8¢¢›?Øm¤`ûv?†"AkZÙ?ŠóÒ'Þ?葉ú˜¦Ä?ŠóÒ'Þ?´¼(&õ;?¨½õ$¡ùN?íhzúêcÙ?¨½õ$¡ùN?T?ŒÔ?J&v•í?o?ïõà9?J&v•í?oPSR4FGL J1406.6-6523¿íúŸpž"ÀÀ
IJFu/WÀ:;Öç‡À;‰5
þÆD@؆V›Ã@,ò;ò–?Ǿw‰ú?L? ƒy`'æi?܉±¤Ó3™@7~'«cœ¿ë; !³ƒû?̤ç«ud0¿é"kaøÃv¿ä¬åÁX¨¿á§@¡/å÷¿ç~Ò£¦bÖOTHERunk1RXS J140629.8-652251?ïù!Ë=é?D€}in'¶?KxӋÔ2®?D€}in'¶?ï܋ì²Æ;?~ÚêbX˜?qº	Ÿbm?~ÚêbX˜?ï³{'{ü?~ð²Ê3°?ƒ!MJJü?~ð²Ê3°?ïì{Û'?K³É–¶£?co"Ґã?K³É–¶£?ï¦`Ìjô?Š‹NÍúf'?†gÌÞc¤Ê?Š‹NÍúf'?ï¡'é6?¯Ünl }?Ÿ+Úú7=?¯Ünl }?î·¯Çû¤?|î×ÓU?¤Žõú»?|î×ÓU?ï+¨Sb9?=2+Šö?šŠÿR$ç?=2+ŠöAGN4FGL J1420.3-6046e?ꝁºÍd?ÎÆŠÖ8À8ÄëVûÀ9CQÀ¼ô@$ýýÇ@œ?ÿºjyñ]¦?x´u4ß5¿Ž€ÚZÿÕä?áÉD6¶Ë@
1iEhêпÁ<õ(áu¦?ÏëIúõÕ¿æž¾°nÈ¿åæŒÇ#? ¿éQ%Â1hX¿¦ÀPë!OTHERPWN3FGL J1420.0-6048HESS J1420-607?ä_âä¹?Óû0ÆOá?×A;ö6?Óû0ÆOá?ﲶ©ò´?£,Ò{Jj?ƒRUºSã?£,Ò{Jj?ä:(V§?´~ŽXüN"?×ý‹¯Sȳ?´~ŽXüN"?ï³¹%%("?€ÞÉ­hB†?ƒ¶²îM%?€ÞÉ­hB†?égôkªÑƒ?È»œÝµ—?Ê`.QT¹ô?È»œÝµ—?î³ú¾wŸt?·èFåg"f?¤ÀTõ¤¾?·èFåg"f?è"3ûk?´)ýãу?ϳu¿0S?´)ýãу?íù+£'À?®i8Oh"G?°6§úÿ?®i8Oh"GAGN4FGL J1423.3-5655?Ý:FÝ"/@
Þ軶$À9ËýíאÀ;€Px@Â.jÑ@´€Ǒ?Ô((}¢˜?á°:Zná_@	3ä%®æ2@9q‡VËê?ï¯oYT/,¿ÞÀ£ô'b¿ê_$º|¿îÚ®/ªè¿ïâô˜VN?ÒÐXþý—OTHERsppSNR G315.1+02.7?ï²j*7®d?¦Â)¹?…?ƒeu€'ÂÎ?¦Â)¹?…?çôÖS‰??Çk>´¾?ÐSXíù?Çk>´¾?ì†óc(]0?¥àô‡v¸?»Èdæ½?¥àô‡v¸?ë»]ç;ãÜ?¤8TP×ae?Áˆcp'?¤8TP×ae?îL2ãØ3?¶Ÿ#yrUà?«<ÑÃ[ÓÉ?¶Ÿ#yrUà?»
qz
.´?Â߃[=F?ìžQоZ)?Â߃[=F?â¬Ë%¾ç˜?¹ÄùÂïÁ?Ú¦i´'0Ð?¹ÄùÂïÁ?Ã)}ðÏ>?²€"+?ë5 ƒÌ0x?²€"+MIXED4FGL J1433.5-5457¿ïÿ÷Å¶@ @¿ã°>À9â2²Ú³?À;šÙ¯3^Ò@)áҏi@5%£þwj?Æ©›o\¯?Ög^~:˜'@Pu-©†w?úX×d«PP?ÀÆtÙpÊ¿ÊýpÄ
`'¿çÇ}³^g¿åWl˜¯ŽÎ¿ëi…ÀçÇ¿ïúñ"l'yOTHERunk1RXS J143329.9-545931?àõD4YÆ<?ƪ<$ڑ?Þw—Ls‡?ƪ<$ڑ?Ö¬%ø¸
"?ÉrW|ø?ä©í£ùo?ÉrW|ø?éži#Òd‰?¬G87yÊä?Ɇ[p¶mÝ?¬G87yÊä?åù½7ÐÉ(?©ÑY!?Ô…^m°?©ÑY!?È»Gdÿš;?ÀGœƒ¦4ª?éÑ.&Àq?ÀGœƒ¦4ª?™‹ˆ÷ÅOÔ?¤¹"QT]/?ï3£¸xÏA?¤¹"QT]/?ÑÓ;bÿ?³ŽÝ£À¬1?çq–bN÷?³ŽÝ£À¬1?±º2éÛ­?˜[g•÷‰Ë?íȹ½P'ú?˜[g•÷‰ËMIXED4FGL J1435.8-6018?ÊÚrvX搿"`Câ'íÀ8†µò•´2À:'s‡Ù~@Wꞙގ@Vžh5s?ÇrªÂ`ã?å.J€¬¸°@÷jrd¡j?þ%J~¬-?êYà[DŸ?˂&¶M.‡¿åŽÓ朂¿ïQ¢£Y6¿ã3*š}£¿ïëÊSuÈÚOTHERsppSNR G315.4-00.3?Ð7…Üùì?Ñé<quc?çä=ƒ
?Ñé<quc?¸àƒÚ\Û¸?²A*g%¶Å?ìãç©?²A*g%¶Å?ÙÌÛ¼eÑ?´€'Ï!›?ã'!Í|—?´€'Ï!›?³¦ð·få?¢JÀ_ÚoÈ?í‹!è÷¿ƒ?¢JÀ_ÚoÈ?¾.µíY¬'?ÄÝñB"s?ì:)BTÊn?ÄÝñB"s?ƒÑ 1ë_â?†P•×ˆ¶Ÿ?ï°¹NP?†P•×ˆ¶Ÿ?ل}ÛŽ?½ŠÎT6c?ã=Ás8÷?½ŠÎT6c?L»ì0¡?PNPYÅ}?ïøüîK?PNPYÅ}PSR4FGL J1441.6-5951c¿âà7Ú{¥Ø?»AV¥O°À9¯ñŸ,ÞÀ;Ld\ ë@î«8}tö@üÂ]Þ?Ñ+L§?ïþ"ƒÕâö@Ù"d¦@Ö m³·¨?ê®=Ë<©Ô¿í'úðÍ¿w%¡'ϱ6¿áY¥-Ã¿ïüwêó(¿ïàzßDH¯OTHERspp3FGL J1441.5-5955cSNR G316.3-00.0?Øq_Ž?ѐÒ~E3?ãÇPq!x?ѐÒ~E3?Ü`íï'?ÎäI
Šód?áωvrl?ÎäI
Šód?àÔµAžc‹?³rPX…Ð?ÞV•|Ã8é?³rPX…Ð?Ѧȧà?'?µY6R!Šê?ç,›¬à??µY6R!Šê?ºá<Ÿ²Q:?Ä»Ÿ9&ùO?ì£Øl	µÙ?Ä»Ÿ9&ùO?®Þ!Ñêv‰?¸;æ¶oø'?î✠h?¸;æ¶oø'?ÏÔ~«ñNÑ?²;
u°ó?è
àU¬L?²;
u°ó?žâ @ô.>?'QŽ~b¥t?ïîþÛn?'QŽ~b¥t0MIXED4FGL J1442.2-6005¿â5M8m¿Á4¾x¡&À8pM'iÒ,À:'_lw! @¡…èÜÎ@Èú½ ßß?½Vx¡k8ø?ÒCf;ô!û@‡ÑÜ×@"Üî^B¿ï§vÑîu?靖¿µ¢¿ã'8Â>Sx¿å"°üŒ®¿ìÒÔMʎ.¿çÐV#ùŒOTHERspp2FGL J1441.6-5956SNR G316.3-00.0?ÞwJsZ"u?ÔE¡LëB?àÄZÆR½Æ?ÔE¡LëB?ÛºF‹2VG?ͳñèßx?â"ܺfÔÜ?ͳñèßx?ÖQ´"#˜?´€°°?ä×%¶rî4?´€°°?ç¾£ÚUˆ?³^Àå|,?Ђ¸KáTï?³^Àå|,?¹ÏŒ«Û¡¸?À€—ÏöÄ?ìÆj"‹É?À€—ÏöÄ?©Kì4£"?µ:5wYs|?îkA<¾ÕÇ?µ:5wYs|?®²c?¯ãc
×´%?ëzœ"Sg9?¯ãc
×´%?·£¹¨Æn?«DWW[¯Ê?íˆÊÇís?«DWW[¯ÊMIXED4FGL J1443.0-6227e?Ò0,ù7ºÀ.>ìÀ9})ž^û8À;ŽÿӊV0@$+Ö²ÿœ-?÷ƒM&ú@?¸Õp_c'Ì?»"™T¥HÏ@X¥H#…@@O~JˆºN¿ïü@ø¨ž¿äpaǛ4¤?ïû
˜	v¡?àÑsZj¯¡¿Ê[Ym¿ÆÞ°zՂOTHERSNRRCW 86?ïýÇQÉÝj?<l1¹¸´?1Ås©vù?<l1¹¸´?ïØñ[ªÿ%?ˆF¤ˆ'?s‡R) •a?ˆF¤ˆ'?ïàdè7?u¼Ù®³Ÿ?oó›3EÔU?u¼Ù®³Ÿ?ïå¤ÖÓO¸?a8ýÖÅ?j[)Ӑ–?a8ýÖÅ?ïú2°s?C•ÝáЪ?Gß6h^fÊ?C•ÝáЪ?ï#É93A?¬ywòø'?›ÕiûÞ?¬ywòø'?ïwºÍ­¾?ßÅ«xò¹?'¦J_¨:?ßÅ«xò¹?ﯯÕúô?'b~¶zŒ?":ǧ?'b~¶zŒAGN4FGL J1449.4-6026¿î|Š(§,ï¿ê]îBhZ\À8ÛM²:zOÀ:dåÏ@"'^±Ž@ºZƒÚ?ӛÍÐeß?ÐÆ÷ µí@ºç"Þ÷r?û…K'Mð¤¿ïÛíÒ?î@œ<âž¿è÷ŸsÎ-ö¿ê^áÂ}=˜¿ìÕl
?ÆhڟsMUOTHERunk1RXS J145023.3-602718?èîa‡m{?ÑtÆFÜïk?ÌFy‰âJ?ÑtÆFÜïk?èíÏYwž?È)[Cµ?ÏÄHš!‡?È)[Cµ?ä–̤w³?¸VK-ìE?×öÒf·š?¸VK-ìE?éaéîµo?°2Ñ˵?ɊxXE*E?°2Ñ˵?ã2ZÅRã?Ðæltâþ?ٛJuçZ9?Ðæltâþ?ÍRze½ý?ÏÕôØsc?è«af¼?ÏÕôØsc?ØùWÆKºz?º9rÒÛY­?ãƒTÚ"Ã?º9rÒÛY­?¼õVvâ¾?±Ooå=*?ìaU1#¨@?±Ooå=*MIXED4FGL J1453.4-5858¿æPÁHµ%'?ÐÏ)~(¤åÀ8ö—¤ÌӃÀ:Z‰%®r@åÀb[>ë@"&~ïÊ?Ëç€Ø,§S?¸MŠÞ|ô?ðx×ÒºL˜@ZÌ´ùòJ¿ÙèyÑ}5¶?ÑUÈôÐ÷Õ¿ç¦G'Jˆ¿èʑž£n°¿ê €¾Z‰¿Ëºzå¤_OTHERsppSNR G318.2+00.1?çí‰è˜ýŠ?Ñ˔[ŸÁ"?Ð$ì.Îì?Ñ˔[ŸÁ"?ï¥äòn®?'©Ó×>Q?††ÃV–	£?'©Ó×>Q?æιK¢$?·Õ$%4~?ÒbhÞ»¸?·Õ$%4~?ï'XԜ=Ó?u~Fêc£K?‹©ÊΡ·k?u~Fêc£K?ãç±­6¯j?Ñì띔ÈF?Ø0œ¥'¡-?Ñì띔ÈF?íŠæÄ0?ÂH5¡«?·û¨Ð'Ñÿ?ÂH5¡«?å}‰yw "?»úR¹WÇ?Õí
¾ø?»úR¹WÇ?êÉ2Q>"™?³†öøYw?ÄÛ6»­?³†öøYwAGN4FGL J1459.0+7140¿ïú?iLtÎ@E
c
'SÀ:*ŒžßS¸À<¿45'²E@"w¡ÍÏ@œSE!rA?´Æ¨à"Xß?²)"ø‹?ö³#ä
Öô@mÆáü3î?ÞKs0yD¿áÁ~_¬bõ¿æ|yÞ=bŒ¿èL÷à 灿ê¯þàÆ(ï¿Ù‡÷%ÛOTHERcss3C 309.1?ïû6qxŠ£?s­}ÛØÅ?C&:Q'ÈK?s­}ÛØÅ?ï÷ãh"	?RoQ§&œå?P9ŵÐü?RoQ§&œå?ïè<kj?j[x°Å¢
?gÃëâµõ?j[x°Å¢
?ïÿcÈñ?1sw8ä?+V¶Œd?1sw8ä?ïýÌaBD?+Í=®;ºè?1œöQa%1?+Í=®;ºè?ïß)	?qÙw~\ir?pk{ûVS›?qÙw~\ir?ïä¯Ñƒ.¸?vû¢wâƒ?kP.oØ+?vû¢wâƒ?ïþï…o§>?Óýš—??!©u²'e?Óýš—?AGN4FGL J1459.0-5819?ÆdàÝÙm?߇ø\rœ«À:Qo'TÀ;ü;ëh™@ÄŽ˜‰¤@9&Ÿ¦ùÔ?Öÿyvƒ??ïÛ>w‰ú@
q#ˆY@,©óXý?î@Ôqü™¿ïÿÏX˜GŠ?ïýP 슿äÉ>$'ý¿ïÿü¿ÙŸC?ïÿ•!îZOTHERunkSNR G318.9+00.4?ã
5hóV?ÑJ=Ô?Ùë•Á.T?ÑJ=Ô?ëår]?¡?ÃÛŚö³H?Àk¦6‹{?ÃÛŚö³H?ésór,Ý?¯IU—2Íb?Ê03¾7LŒ?¯IU—2Íb?æ>~ù¸Æ¹?¿‡ìU©?ӃŽrŽ?¿‡ìU©?ÒMÉDŠ§?ÑoŒ‰‰è?æÙ]º¬u?ÑoŒ‰‰è?ۊA…d ?Ó!7?(×1?â:ß=Múp?Ó!7?(×1?àpC}?À¤Áííü?ßÁéyÿ?À¤Áííü?ÒÍïT¿¨€?ÅgUnòQ?æ™U +À?ÅgUnòQ	MIXED4FGL J1501.2-6624?Ó䏃ÛÀ÷ /µÐ1À:Óúœé°2À</†K<@F6­;7@³©ìiJ?ʈüˆý?²¬¿¼°?ì‰8ž2Z?ÿ<¾U¼u?çåWr­œ†?é:ÂG¸¦¿é6Ä¢–¿åË·Ä'Þ¿R'4wU÷Ù¿ïü« —OTHERunk1RXS J150054.2-662400?ïöµ¤AÇ?|4Né(—^?R"·}Gbò?|4Né(—^?ï×
²½yj?ƒ EÝ;?ty&¼>Í?ƒ EÝ;?ïʘ©øY?|±Kö¬Ò?z³öæ˲?|±Kö¬Ò?ïòÄÒÃ?HB™€|#?Zv['§•?HB™€|#?ïÞ3¸qK?xjߢÓ?pæ~÷æy?xjߢÓ?ï	­€D¹?±‹û͇?žÊOîšß?±‹û͇?ïcoò½]?'Ù°óÃÕ¯?"'­{º?'Ù°óÃÕ¯?ïŽSò4T4?ƒßc²<â¹?Œk}9ÆÞ?ƒßc²<â¹AGN4FGL J1503.6-4146?ß)ºâG;@->X¡UPÀ:ôx'Y
]À<_JÚåª@ <','Û@éLz,	?ÉVöœT	?'Ÿk¯j?É,{Éz?ýH=ägF?$_öŠ¶¿èfÊo${
¿rÈÕ`3
]¿çÛêw¿¿àŽn—€¿à`Ý?á—_OTHERspp1FGL J1501.6-4204SNR G327.6+14.6?ïûÔÕ.ñ?6è'ɦ?@¬«œ1îŸ?6è'ɦ?ï×\R'Gf?€Ç­»»¨?tQÖι¥?€Ç­»»¨?ïᾓùòu?sBI9N'?nAl
-(?sBI9N'?ïçWrá&ª?Oõ‹4_ƒÍ?h¨PS¶&?Oõ‹4_ƒÍ?ïùp6ýJÍ?B@¼è}l«?J?#´…´?B@¼è}l«?ï(|'ÔÓy?§:C-2Zt?šðo¬DÈÛ?§:C-2Zt?ïÛû›í0ð?xΈç‹?r1ÿ³Ý?xΈç‹?ï'lsh#ø?y°˜•ãِ?‹dãÊ?y°˜•ãِAGN4FGL J1508.9-4110¿ä´ MÓG@-F§&J¥À:ÝÿTßUfÀ<'…o@*@Kڔáy@ñã݊Š?Ò'™¢ÓÕ?è~è]¡ñ­@¶,ºs-õ@y,¼¡†?ï)'Dé>¿ÒփDm˜4¿à(֞椿í'Í+d2¿ïÿß^IâL?¼ð&n(҇OTHERsppSNR G330.0+15.0?â¥=,Âfþ?Ì"?Úµ…¦{2?Ì"?ޞVÁœ†Î?Ëòvv?à°ÔŸ1¼™?Ëòvv?å#¾p¾"
?²ƒë7•b?Õ¸ƒ'÷í?²ƒë7•b?å~öy0)?®ï1":?Õß
Ÿ®?®ï1":?Á\A´Ö6?Á9çØ@ô<?ë¨ï'Êr?Á9çØ@ô<?©<žãLÄh?¶\ºä>™É?îl6½uJ?¶\ºä>™É?ɛJ;ëò
?¯Ë8ìéIq?é™-q~?¯Ë8ìéIq?·RFõ
ä?¡È—"B'?í·!iÝ?¡È—"B'MIXED4FGL J1514.2-5909e?ïÙāq&*¿óW"ëïyÀ7§È‡Ã®@À:ä¥Xê|á@!Á»¤[iˆ?ý<96's? ›ªãÔ?s©…ž/Ãw?яãÉén@KûXÑRn¿æVc"3Öǿ䭕X¥´¿åÌeÔp/=¿ÔuÜyh¿ßÍ܁˜¡¿É(èÁõÙ6OTHERPWN3FGL J1514.0-5915eMSH 15-52?ïúµ"?ƒ/ÙÑü?aqVøëÔÇ?ƒ/ÙÑü?ï՛ú‹»¤?'!‡4[?u2ÖNù´?'!‡4[?ìefÈЭœ?§­¡Æ0Gé?¼Ôɹz""?§­¡Æ0Gé?ïwtžÀþk?‰‰NWWÔ?'l)˜?‰‰NWWÔ?ïÇüPz?{'¸Ç­¹A?|wþ‡®Ú?{'¸Ç­¹A?ï1ðŒ‰T—?¬W
Òç¥?™ÁînÕm'?¬W
Òç¥?íIª¢š8?¦Ï¶|¢i¬?µ²ªêRXb?¦Ï¶|¢i¬?î3æWÉ{Æ?©(ÛÀ€oC?¬Áš… £?©(ÛÀ€oCAGN4FGL J1518.8+0203¿ç‰ Ýñr@G]{á!îÀ:¯c>"¹†À<bã¹x\2@NóÄÞ@è@,¢Ûa»?Ð2&ìS?Ýï!‹k@Û·-[@9È"Ãú@¿ïÿýF\I?ïÿíUÙPi¿à%>þÃj¿çÑt!N¿ëçÇ$_¾¿ïRþª•jOTHERglcNGC 5904?íê{GZBÓ?À•‡¾?°¬%ÄRk?À•‡¾?íFqðÌö?¼ÁòíâŠé?µÌpxNux?¼ÁòíâŠé?ëØ
ârô?¥ù•#º±?ÀŸÔw¢4.?¥ù•#º±?êÐRd*A?£šÕå^ ?ľ¶oÏVü?£šÕå^ ?êÞ½f±?Á(¶'Vb?ą
d÷•<?Á(¶'Vb?ãB‹.- 0?ӃÊ~­žÎ?Ùz飥¿ ?ӃÊ~­žÎ?ç¯mbÑRæ?³\R&­-?С%:]Z4?³\R&­-?ÙR­,ڏ¿?»PÿŒg¬â?ãV©i'¸ ?»PÿŒg¬âMIXED4FGL J1528.4-6729¿ïúéâÿŒÀ"X%[À:·ä‡ÔuÀ<qfŠx"f@!
Œ!¶Þú?ü¢î¬ñe3?ÈZKæ]l˜?¿ä†Ò… ?ú0– ÀÕH?ö¿Ê"xzæ?ïþŽø›ˆ¿ÝLr^í T¿ãÜT)M¿Ñ¹Á¢w8ǿݬðäY0s¿á$I@:ؙOTHERunk1RXS J152815.0-673003?ïýWc`™ë?1̎P]?5Dä$î;?1̎P]?ï˜Doú?›ä
Î]?‰îãú›$$?›ä
Î]?ïヸ[э?lm{|LՏ?l|Gx3sB?lm{|LՏ?ï–9A.r?kTÁc
Fµ?Šq¯¦¾s­?kTÁc
Fµ?ïùò¨å£?L^•í«?H5]
Ô'?L^•í«?î"°ÃÏ?¸ðO6Ë£j?¯Äôžõd?¸ðO6Ë£j?ïÇp«ÓqÆ?€«FփMá?|Gª2sè¬?€«FփMá?íx–ŒãË?›Ph}`á"?´;O»*î(?›Ph}`á"AGN4FGL J1533.9-5712e¿ïÿYõ׿ïÿ"ÞïÀ:°ßé	CvÀ;s­íät‰@(ŽÂ¦]¨?òUav<??ÕÂZµX<?´–ÜO÷?â	>m#
?ô´ù[öö¿ïÜb¦-¿ílÚ>$}ä?픁+äŠY?ï÷ÂCÜΣ¿ä*X-¾,?Æ%{º‹©OTHERSNRHESS J1534-571?ïý!xe0?M'‰†?6ó'j?M'‰†?ïSɨ·?µ@Y=\M?•†åaï?µ@Y=\M?ïˆØCð½?‹ª³E²Ô¹?ÿIòsl¸?‹ª³E²Ô¹?ïU!n~|¢?—ã´šÊô?•[Ò+	×?—ã´šÊô?ïýK!Äÿ?8¯Ûøÿ?3õ¦ü¿m?8¯Ûøÿ?î\ºKüéÜ?¾ZXóÙxy?ª4[BÅ9?¾ZXóÙxy?îӚ"-ˆ"?›(aí=­?¢ÆVÎ]Ì?›(aí=­?퉗ÅrÕ#?¶[ ±'44?³³AÖ!$â?¶[ ±'44AGN4FGL J1534.7+2331?à¬uG"@J‰,à2ÛÀ:rÚ:s™UÀ<t¥µ0Ï@£àE$¢L@YÚakU?¾/$…ÆS¿ƒ@f«
gû?ÁÃì¾Ú›Â@y͸/0ð?™t6!"èD¿åaþÝÁ׿ä]`='l¿æ·a*½Bì¿èÀ0§g¸v¿³XƒàÛޟOTHERsbgArp 220?ïùУ*?KH€RÐ?H¿Þý`€ì?KH€RÐ?ïöÒÜJ2?Z;¤Á¡è¡?RZGïŒÑ?Z;¤Á¡è¡?ïäQò'?nùÊÍ<`?ká®	ØæÊ?nùÊÍ<`?ïóh$"•?BߑYÂ?Y/¶‰cöZ?BߑYÂ?ïÖP¶¾B?qmN4Zîk?tפ悗&?qmN4Zîk?ïÔ|Á>º?€éšÒ˜'‡?uÁŸ~F»?€éšÒ˜'‡?ïÇ¡åÌ?¯Óó'Ć?|t.÷€6?¯Óó'Ć?ïʙzÔ¡F?fþý^€?z³B/üà?fþý^€AGN4FGL J1544.5-1126¿ØÙ'ê7@@9&A³À9=ì0?bìÀ;ÈRÆvq@âd¬'ä@5†S€?µaL̆Ç?ͽyȘá@ºx)‰‡?ú¡®÷Š?ïÞðáT[¿Úiþ Õ®¿å®í¾´Ü¿êy…'ͼ¿êlH"ș¿ïɞs`JOTHERlmb3FGL J1544.6-11251RXS J154439.4-112820?翦u9ì?ÍÓ=ÁÎäL?Ѐ³þ'?ÍÓ=ÁÎäL?ßG©'_?̒¦ÜßOÂ?à\p+>Ñ?̒¦ÜßOÂ?ê™dâÐÆ?ªÙå£p_?Ślt¿¼æ?ªÙå£p_?ã!¹!¸ü$?³X÷!"ÿ"?Ù¼¼Ž·?³X÷!"ÿ"?§,â¶`?Âc.k?ëV4ÇRh?Âc.k?½!Ýd8}?¦Š\B?ì[ÄSxðN?¦Š\B?Õu-VØÝZ?¶vì…Ä?åEiT"'S?¶vì…Ä?µ8ƒ.ÕÖ?¤ç%·¡L?íXïšN—µ?¤ç%·¡LMIXED4FGL J1545.0-6642?§t[ä°­ØÀ"ÃH² yÀ:L÷z€ÏÀ<Kµëæ@"!N"b£
?úÅva†,Õ?¾dZGŸ&?™p1ãŸCŸ?Ü˞":ê?ýà¸L7;+?ïöD_«aB¿ìáT™4¿áW'ÏQâK¿ÕHd]L·>¿ÃLu9_¿Øõ…ÞPضOTHERunk3FGL J1545.0-66411RXS J154458.3-664153?ïü+˜â´??¨àÓÙ}?>£>•`F??¨àÓÙ}?ïêæ<×Ä?xŽ2½cñ?eÃ>9fË?xŽ2½cñ?ïð‰œî°?_x­ð¤Ô?^ìƞQ½¢?_x­ð¤Ô?ïógKœ>B?CM3úxÆ?Y1i2·Jú?CM3úxÆ?ïøe&âg?D2Ú¾#¹˜?Nkg•½†?D2Ú¾#¹˜?ﭞïCð?™\ÑR¦?"˜D5ã1€?™\ÑR¦?ïð5»´Ý©?izª?×úß?_"ˆ6ž"?izª?×úß?ïфÕÅÍ]?i4­"áô?w=•º¹­?i4­"áôAGN4FGL J1547.6-6601?ä!w
<]ÃÀ"ì·M߇À:¤W‰SÑ8À<òÙ¦Ïã@k\æàÊ0@¥2.?Ézô'äs²?±óy^æ•K?é—tü+@áZº5Æ`¿ì"Ö@éÕ?ï÷_²íþv¿í°Ú'ÿ#¿Ô)ªžNµ¿ïþ;âÐ?ïÚÑrMû6OTHERunk1RXS J154730.5-655754?ïñFçù"?`tkKÐ?]r068'7?`tkKÐ?ïä«
…??z\/ÎsCÛ?kTõhâî}?z\/ÎsCÛ?ït»^˜ð/?‡M˜ÃÈ?'h"+*,"?‡M˜ÃÈ?ïõÂ2?DŠŸÅ"¬¾?Uâ|´Ù?DŠŸÅ"¬¾?ï°E™"Œƒ?ˆ
ímE¤?ƒî™¼Ü?3?ˆ
ímE¤?ï/ç˜ç(?°Ùv[—y†?šÃãö?°Ùv[—y†?îûëz.g?–%üѽÆv? NEÉd˜?–%üѽÆv?ïƒU;Š‰u?"ñnβ±?*±~jÁ?"ñnβ±AGN4FGL J1552.4-5612e?ë͏¢AUW¿ûöŸ™ÛÀ9Ü'³£0À:úZiØá®@!8X"UëD?ý¹á7½Üo?Á=
w}:?ÅÀ=\×ÇR@º.šG>ƒ?ó/ëb^?ïÿÔač¿ïèë Í?ï1}ñf®¿ÚTÁÔiy¿à&ǟ¼Hp¿æÞ'h#ÕÈOTHERPWN1FGL J1552.4-5609MSH 15-56?ï/2éÈlQ?²Ê båÂ?š¢ÁËä?²Ê båÂ?ç§~›Þº­?Ë,­tº3?бÈBŠ¥?Ë,­tº3?íB‹ªºöƒ?¥w›€?µë¢©ºXi?¥w›€?åêè·öG?·[ûâx«n?Ô*.çq?·[ûâx«n?í€cøy?´Kë
nl?³üà=ê\°?´Kë
nl?ÓQ£üt_?іó%jâf?æW.ÅýÑ?іó%jâf?ê¢ýèÅô?±eH¨<)?ÇÑt\è0?±eH¨<)?ÑF/DZš?ÁJ.ëè?ç\è?]Ò³?ÁJ.ëèMIXED4FGL J1552.9-5607e?ícýéqÁ¿ûÃ"›5{À7ª·Üz¿ºÀ:RŽ¨¤ÏX@ –=^…F{@¿Å¥'¡?«`Þ"J?µ(™QJJ|@È7 €=¨?ôý>!MØ{¿ä©»Þh?ïÿ—Ôú¿âJq=Yý¢¿ÞF™!N¯;¿äÒ,ó~~¿ßŸ[O7OTHERSNR3FGL J1552.9-5610MSH 15-56?â0ƒœhg.?ÓBúF鯘?۞øÇ/1¤?ÓBúF鯘?Ô¢L÷æ',?ÊÀ‡W€M ?å®Ù"¶ê?ÊÀ‡W€M ?㒠ê@%?¶	/ÑðFP?ØÚ¿ú+¶?¶	/ÑðFP?Õ'™^ªA?¶¿(}'¹?ål3|Pªà?¶¿(}'¹?à{êИß?ÒÙQIJÐ?ß	ô*^ÎB?ÒÙQIJÐ?¥Ž7¨È<™?±ŽÏr5Õä?WÿW?±ŽÏr5Õä?çû°"ºí?··\Iå¤?Оö‹ô&?··\Iå¤?™"@´1=?‰€•é@?ï6ïEÑ#&?‰€•é@MIXED4FGL J1556.0-4713?é™MâiŸ´@EUÅ.rÚÀ9F"'AiÀ;.…bªð@Èӌ.¡ÿ@K¼±Ì–F?¼ueáÙ?™:†¨j?܁M½£7?ä;CÖw#+?ïÿý{ÁA~¿á[?÷fÔJ¿ëwpåEi—¿èVÇ¡Р¿àãÕÈc¿Ô‡^ƒ˜üOTHERunk1RXS J155608.6-471529?ïïÔ|^?hD29ÜO?`+ðî?hD29ÜO?ì¥Hÿ£8Õ?½šWss.?ºÕ¸æ9Z?½šWss.?îÒÕNóÐi?•Öˆ2J\?¢Ò«wvs?•Öˆ2J\?í½påV—£?š)ßáø9)?²xÔhn?š)ßáø9)?ïH"QšÂ?ŸyDU­·?–ïu̾g¸?ŸyDU­·?×°Ùd?ÒMÀ}Å9?ä'"upÍü?ÒMÀ}Å9?íÞ¡C:? ÊEG­Ÿ¨?±
õè<#y? ÊEG­Ÿ¨?ÝÚb¯–9?Á>UnO¥?áÎÀ(4ä?Á>UnO¥MIXED4FGL J1601.3-5224¿ïL/lîڃ?ÔÓëd'{ÃÀ7øKZqežÀ9ÀBHyìU@^¾†GW@løÿZ¾'?Ã÷ÁÃuU?ßó†?IÁë@ÖO@¯óx?úŠ9\mT?ïìz|àP¿Ñ¾²m{¿èYüá¨I¿íhåf÷…Þ¿ëf`ۍ¿ïäèaþ¢³OTHERsppSNR G329.7+00.4?ÙÝ3™­?Ôp¥€=ä"?ã}t'f3*?Ôp¥€=ä"?»7gd,?µ'\J­ò?ìœ9z~?µ'\J­ò?ÙÂ@èä—?¶#,Nh¥?ãxߋµ?¶#,Nh¥?£úÚûYj9?ŽMyai;?îÀRP.ì}?ŽMyai;?߶ÇvõÖ?ٙVôê‰\?à$œwD…?ٙVôê‰\?†\VD9©?‹9àõ™aË?憐–‹r:?‹9àõ™aË?ÍÐÕE`?³¬HÏ{Í?è¿KÊ®ºh?³¬HÏ{Í?7ð·r?0[X&¼k?ïýb&÷Í?0[X&¼kPSR4FGL J1615.3-5146e?Ì ä(g¿å3X ÈÀ7ØÏä¯A¢À:o]Ø"ke@#.zìu†?ú#'ǁ&?²¶""Ý?º ~"¿÷@
\irŠa?÷œŠÂ¼'¹?ëWË-\¿ï";C¢í?ïž%"ôÆç¿Éf8ِT¡¿×æø<g9u¿Í)- Í›OTHERSNR3FGL J1615.3-5146eHESS J1614-518?镣cOŽ;?Î5Q?É©rrÁÇ?Î5Q?è ãd`I8?Ï£¢µ²?Ï|rn~Û?Ï£¢µ²?å`¿¨%'?´µ¤$?Õ>Â¯´Û?´µ¤$?ãqGd‡Wç?ÁP—û'e¦?Ùq6ñP1?ÁP—û'e¦?ìçáÀqA-?¾µ®<Ò­?¸Àñûš—?¾µ®<Ò­?Ü'ûÁÖµ?Ԕ^™{?áìr"¦?Ԕ^™{?èt'ojb?·ƒÿœùb'?Î-¶BWúy?·ƒÿœùb'?оÁ"½ðD?Ãô]PyP_?砟5¡Þ?Ãô]PyP_MIXED4FGL J1616.2-5054e?阶ÝC´Ø¿À©ˆOnÀ6â1_ô\^À9ÎÒÿì´Ê@!®š‡«/™@aED­®ú?¡Ùt~Þ$?'¾#3-K_?á¡_²??ühˆ_?îï«>\²?~c45oV-¿àŽ·ó÷´¿à"pð›¿äÓgÁ¿×‹&ŸÇ±OTHERPWN3FGL J1616.2-5054eHESS J1616-508?䇚ó$¿?ÑÛZîõ'?ÖðʶÔ?ÑÛZîõ'?îL½9ÿ!«?½/ùh^†?«4,dYhI?½/ùh^†?ã¤h;R¼?´Tèó³'I?Ø·É/‰Z‡?´Tèó³'I?éq׳°œ?¾îiƒë÷#?˶8¡1=?¾îiƒë÷#?ãÚékF¨?ÐßJP¹´u?ØJ-)r®ã?ÐßJP¹´u?ìE*>öh…?È{x¯œÃÎ?½Ö®L»×?È{x¯œÃÎ?çȉNó®?¸«¤zäœ?ÐoÖíb¤?¸«¤zäœ?ß^•üDù?ȉVLь?àvPµ݃?ȉVLьMIXED4FGL J1616.9-2257?åç)"ŸMt@3|€Ç:¼"À:GOµò–À<	÷´#ì@<r¢ÿ@gy¦µ?ǔf'?Õº´|ª@Ú<÷Ø?üdî—!ð?ï÷n@ÐT¿ät<Ëbj¿ßÔ½|Lן¿ßͺ}¿ÉY¿îZŽâ™¿ïÿÿ)@k*OTHERglc3FGL J1616.8-2300M 80?á7×Óø t?Êgw=	‡?ݐPX¿?Êgw=	‡?â¾VƒU›¤?ʚš{ýã?ڃRùTȸ?ʚš{ýã?蚐Þù¹Ú?°u§®d"Æ?͕¼"š?°u§®d"Æ?é?_Ö??¤¨ŠWš6F?ˏ€§Ÿ?¤¨ŠWš6F?à‹ø®ýÙà?әÎû¸À?Þè¢L@?әÎû¸À?¼úꛮ‹ˆ?ÃË/vʦ?ì`¢¬Š.?ÃË/vʦ?Òr'S5B?¹p_Î+N?æüÆ·Ve_?¹p_Î+N?ͤ{RL—?«$­Ù "?è–á+\,Ú?«$­Ù "MIXED4FGL J1619.8-6314¿ìÕضSÓVÀ"‹<æÀ"À;N»"¥íÀ<¤$Ÿòy@!ŠÙb\k'?öhó ¸r?ÖuK[žn?Úû•!ººÑ?ù¢aôçž	@µ'§‡ÃÙ?ïŽ^g"cпíÉ_²¿êsŸ¿£n…?á¹O!P\º¿Ùâ`ûÈ¿âU1U¡ÏOTHERunk1RXS J161946.9-631530?ïðxÓË«?žÛ¤z
D?_þ]è
d?žÛ¤z
D?ïéæÊ5)?yrNëº<–?f6¯äÐ?yrNëº<–?ï½O††–?z*Y^òÓ?€¬{ö‡?z*Y^òÓ?ïún6œ'?4{2êö\?FG³N=÷:?4{2êö\?ïõÇ-Kí?X$°+ˆò;?Tq¦&•	?X$°+ˆò;?ï"'Û¢cÔ?¡}8&Ap(?Šö	(•õ?¡}8&Ap(?磌öϐÞ?‡-'ü‹?…U>]X­?‡-'ü‹?ïìÕÆø?]!3©í#*?c*9ïJà(?]!3©í#*AGN4FGL J1626.1-5904?åÏò¾p`À¢	?Câ®À:Ûõ ¨ìôÀ<ªŒ0$‹@ Xs~@©ñ…é¹m?Ãé§c†¸¿¦±€Á™G?è<ÓÅåR@ïÃåG—ï?ïÓýB¶]õ¿Ü¬3$D­Ú¿ëÓ	\ ¿èw~¶ß%¿Èäß¾%±?–''ᶶ,OTHERunk1RXS J162613.6-590658?ïù2êÊ?oävex±î?K4U|ò?oävex±î?ïè6WªáÀ?z'd=WQˆ?gɨ%·É?z'd=WQˆ?ï̐ª2?xddøt?yör$m:?xddøt?ïüð.âÒ¯?'1Îì<+?8~ŠïI@y?'1Îì<+?ïây¸¹ÖŒ?oÔ…0Ó?m†G0+óú?oÔ…0Ó?ït··^H?£wh&Ù?'i	ÎÌ?£wh&Ù?ïŠäv¦iP?Š}ÕÖ§:C?FâH§<.?Š}ÕÖ§:C?ïÞ:¡^?j"÷ÝÇá?pôâ—C»Ý?j"÷ÝÇáAGN4FGL J1626.9-2431e?×Bׁ—Ö\@0º{¢7ÍÍÀ8.ΉenðÀ:¾É'•q@ÅÍc ŽU@ÌՀÐtø?°ú*~å8?ºãi`/¯_@šÐ=š•B@oXiM¡t?ï¦qï0¤ã¿ÚðŽ•·¿å,¡^4׿äL-ráõ¿æj#?O§¿ì½¸ƒi¬OTHERSFR3FGL J1626.2-2428crho Ophiuchi?ïÉÆचÿ?ƒHÁž¸–?{µñ:?ƒHÁž¸–?ë"åF‡,?¾yI·3?Á¬k¶åãR?¾yI·3?íöS¡¾?§f´" pö?·xOެ̑?§f´" pö?í
ó‹R"?˜X6•?·c¥ÙÓL?˜X6•?ïüO‹m?¡amq1@v? vÃÜW?¡amq1@v?Úæ]äÚ5?ЂoIA›	?âŒÑ
'ÿe?ЂoIA›	?ë×áÕêÐ?¬£ëöp™?À x¨T¿Â?¬£ëöp™?Ü©ùº&é	?¹dpCôq?á«"ì‹{?¹dpCôqMIXED4FGL J1627.6-3852¿ïß[Öљ¡@²Y@ãõÞÀ9£.>׬$À;‡A©î{s@•Í`E@¨@ƒ}Îb?Á7úÃ*6µ?Àž}5ês?þ•Âú»óa@8þ'¢?ïþ0O‹Y?½ï¦–'7þ¿äAç`ÌÉr¿åYg°ã¿è›lØpnþ¿ßgÍÚmOTHERglcNGC 6139?ïæX÷4vÍ?xµø…mŽ?i§Ì?xµø…mŽ?ï†ËÌÌå?'Òc7þa)?ŽMò-ŽÁ?'Òc7þa)?˳>©?‡ËGb?Šž
0UÖ?‡ËGb?ï†+`+
ö?prä}àVö?Žu(úò?prä}àVö?ìõH¨'?¹c«~§–?¸U¿'Qør?¹c«~§–?ìˆËAB¦ª?¿{Õ#–ø?»¹¥õêʱ?¿{Õ#–ø?ë=Ü?Ÿ?´.åÿ¸WV?Ïõ…?´.åÿ¸WV?ìÇwýd]? К#I?¹Ä@ôÝ? К#IAGN4FGL J1628.2-4848c¿ãa(µ£2¿§¦{ªEÀ8ɦ¤D‡À:>žm=ðü@7RÅʤÿ@±y|ßý?ʦE9'ô?Ûß°i¿·;@'mŸ?ËÈ?ø2·bWc¿ïM:'£?ï­¨z-¿ÃœÏÄxëN¿étæX¿î¦\?ñÝ}¿áì!%êuOTHERspp3FGL J1628.9-4852SNR G335.2+00.1?ÓÀïû6Rß?ѵ"gš)H?æˆd֑?ѵ"gš)H?ÈÈ ~Õ?"d\åð?éÍùy—àK?"d\åð?ØJœ{¡6?¸×|úJ¶?ãÚ±Â/dò?¸×|úJ¶?Çúã(·aß?ª'ý?œ¨6?êG5Ò'ˆ?ª'ý?œ¨6?¤¿+¹í!+?³Ÿïý‡y?î´
D¥æ?³Ÿïý‡y?'îDÊ=?š=ÿ§Ûö?ïpÙi_·?š=ÿ§Ûö?°}zÒt¥›?ž%µ4&?íðP¥èe?ž%µ4&?uÌv\Ë?hw¢²Ÿµu?ïÔg4?hw¢²Ÿµu*PSR4FGL J1630.2-4347?ïc–H½oH@	ƒÏ:eVœÀ9ÓT&ÈÁ¥À:ý¿;ÒE@ )f*×D@«Ænäº?À8ò9î¹1¿²ÉÖù "?óu­+FÕ§?þZ¿êU?ïÿu+%G¸¿èZ&–m¿êzÿzŸ¿éŽ!€Ù.Z¿ïá0œýç?ï"Ic `ÉOTHERunk3FGL J1630.3-43461RXS J163023.2-434804?ïŘ;(R¸?ƒ½PÍáÁo?}3âUÙ$?ƒ½PÍáÁo?ïɋ#à?§‹D.g£?FΒìùŠ?§‹D.g£?í ÒMjA?¡‡f@o¿}?²ùm•÷Ñó?¡‡f@o¿}?ï £@·UA?v+='ù"Q?‡×/ßé™?v+='ù"Q?ì5 áÀ–?¿e$Nõî?¾RøñÿóQ?¿e$Nõî?çîˌ}HÍ?Î%uÊ cç?Ð"hçne?Î%uÊ cç?셿Á×?¦7=Òöü?»Ò÷ÉG)?¦7=Òöü?꓇Œ¯Xü?¶n@&@?űáÍBœ?¶n@&@AGN4FGL J1631.6-4756e¿ïÝ@àšßë?Å>ÜIA'rÀ8;i÷ë^ˆÀ:,žh5s@#‡QàG}î?ü°œ!3?³¬
åpݎ¿›äÚ5+¨? ®¡>@c#ÃԀ ?ïÍÐmk=f¿ïý·áXJ?ïh_/:€/¿â;&a"˜Ï¿Ü³±ÇP·¿Ã•Ýað_úOTHERpwn3FGL J1633.0-4746eHESS J1632-478?æÁñ±M?ÐÁZ—"ö?Ò}Íþg?ÐÁZ—"ö?ïÁ	fŸàõ?–xƒ4#û?{L¡¡)v?–xƒ4#û?æ'-q¨8ï?¶íVû9q¼?Òû¥¯Ž#?¶íVû9q¼?ïtžÈ?‰uØ]ø?'l<¥^(?‰uØ]ø?ë!"z|??ÃuBwÒä?Ãyï'?ÃuBwÒä?î÷8;ãÀ?°Þ꣘? Œ|LB(
?°Þ꣘?èóžº.©P?¶æÎ 		ê?Ì1…EZÂ?¶æÎ 		ê?î•Ó±øŽ?¤Ùè+$)?¦¢ÄíX©'?¤Ùè+$)AGN4FGL J1633.0-4746e¿íÓql(ó?½Ü—Æ܉À6 þÊuÚxÀ8öÇÿ²|@ ìÒ1æ'@éÓHæ#?¥Ž
¢ÎÕ?®ôßô5¶@'Óh@bëà8du?Ü`àjcv?í¸Dµ;¶¿â_{l‡é¿â£-ab§¿äÜ(ŸÜSÓ¿âù ÀTnOTHERspp3FGL J1633.0-4746eHESS J1632-478?Úݓ>5ŵ?Ô¾9®nà?â'6`å&?Ô¾9®nà?ärÎ^ûÁ‹?ÒKí㷎¼?×cB|ë?ÒKí㷎¼?ãÄ9Ë}ÂN?´FŠy9S"?ØwŒi{e?´FŠy9S"?ß6ðhCœs?ÁLVÐqG?àd‡ËÞ1Æ?ÁLVÐqG?ãQþ°¨1–?ё¨™'¶÷?Ù\ž¯œÕ?ё¨™'¶÷?Ô`MÎü
=?ÒX;üì‹j?åÏفùa?ÒX;üì‹j?èk4Êj¥n?µ€EXÑ\¼?ÎS,ÖUjH?µ€EXÑ\¼?´á"ÂwÛÅ?°!'©w?íc͇‡É8?°!'©wMIXED4FGL J1636.3-4731e¿ã8äë|I¿¿t Ù¬"À7:¯ÿ6¬À9b>G]@ …†× @t[¡çEõ?¬û&Qxm¥?»%A>IøÙ@Û]9—?ÿ=lP‹3?êv?ø="ß¿×Á±[Xp¿å9‡
Jݿ䧤WÚ¿æç: ã$}¿é
ŠA·ÛNOTHERSNR3FGL J1636.2-4734SNR G337.0-00.1?Ðek'b¤?Ð1ÞZ¤øY?çÍ}J>ή?Ð1ÞZ¤øY?ÔEýVµø?ÌOuýé5?åÝxT¥?ÌOuýé5?àHµÊìfµ?µÍúx-m‰?ßn"j'2–?µÍúx-m‰?Ðt3¨ñ3?´WÀìzÚ??çÅæ+÷g?´WÀìzÚ??ÕfŽ&@Rù?Ð]Ú|ÉæO?åL¸ìßք?Ð]Ú|ÉæO?£I

õñA?³C~fn#?îËo_^_\?³C~fn#?ä««nЏœ?· BÏØG?Ö¨©"^àÇ?· BÏØG?…s»x6~‰?}ÇmùhóE?ïª1,äv?}ÇmùhóEMIXED4FGL J1638.5-4657c?£õ+A6¿™¬.FºN›À7´Ñk—ÿÀ9*OTÑél@ ¹ñ¨ÏB@H½Þó?þ?½¨K
DŒ!?ËE‹:_e@ŸwÞ]îÉ@^ìJìbi?îelZþ¿ä(05Qñd¿âý™ô2l¿æRɛ¿ä‡¿ê²á~µ'ž¿ïÕ)ÝÉõ,OTHERspp3FGL J1638.6-4654SNR G337.8-00.1?½¿J÷'ÇÎ?Æ!bê¹?ìH¡?Æ!bê¹?ÔSðق£ð?̼½yâ]ò?åÖ">®?̼½yâ]ò?Øu6Ÿ	¬?´Ì÷1À»s?ãÿEd°{*?´Ì÷1À»s?Ù•Õ?»Øõ1gS?ãpøxw5?»Øõ1gS?¡K¬†Mù?³AúÖ÷?îëE7¹ø?³AúÖ÷?¡­¹;ipY?±—îä°¶o?îå$lo;?±—îä°¶o?¹Ì´#2µ	?ª‡*?ìÆi{™©_?ª‡*?‹À8×ÇX˜?…ÏOԖª-?ïÿ¼_}?…ÏOԖª- PSR4FGL J1640.6-4632?áy'ËçA¿•aÛížvÀ82]œ"IÀ:n­2ӑã@#L¥)DÇÛ?ým  ôØ?±š!(ïl?˜Aä&Ìn?àïJÀîr9@	'™oþ?澖stkã?äK'Iñ»š¿àsuã±ë ¿Þ_ÂWÿ¿áLʳíض¿½VtUè>îOTHERspp3FGL J1640.4-4634cSNR G338.3-0.0?ì>z—ì¯?Âìê#ŸÂ?¾+Gš…?Âìê#ŸÂ?ïóД$?žäÝ ë® ?ˆƒÍ8Ž"?žäÝ ë® ?ç]¬G`?¶jŒ\aƒ<?Ñ×D§q@?¶jŒ\aƒ<?îü¡ä÷?•4¶"Fáu? >%êö-™?•4¶"Fáu?ì¥Ð¸OùN?¿|±_º@?ºÑz=€5'?¿|±_º@?î¡88Dƒ×?´˜³*§Wú?¥ì|y$
Ž?´˜³*§Wú?éMýcîg?ºOwnmé4?˪È
pFd?ºOwnmé4?ìu¬4ÚZÝ?²náÁæ:?¼RžY-)?²náÁæ:AGN4FGL J1641.0-4619?æ *®ý¯?´J b5ª1À7rÀCQŽhÀ9hÞZ"Ê@Œ‰G.=@•&§3¶?±B€Ùfè?Ã%>¨Ý.o@¾Oá¿£@ø»h {?ïþ/°Ç³ˆ¿á°"Ýz™ú¿âžÝ¦8äM¿æ…~†T¿êDûbÓ¿ç|VÈc±€OTHERspp3FGL J1641.1-4619cSNR G338.5+00.1?ÇWÖý8‹ž?Ì4! †?ê*
@±Ý?Ì4! †?Ôqçk "?Ë«>¡%?åÇJï¾?Ë«>¡%?ÙÁO:Ý?·¸EI\?ãXvtâ'?·¸EI\?Óé–Yü©<?´…‹ž…ñÚ?æ4Ó«b?´…‹ž…ñÚ?·¤Æe?úá?ÁáWø~ED?íg3.ÅT?ÁáWø~ED?¡ïkH¨"Q?±_³W¦r*?îá	K>}û?±_³W¦r*?×È]PVôG?¶ÄsÙ]Ø7?äÑWԅÜ?¶ÄsÙ]Ø7?‡–Ùå}âs?}ԑÑn?˜®À¦?}ԑÑnPSR4FGL J1641.3-5945¿´l¥ŠÊ'À!›ÿCAžÀ:Jœúw*À<ëoOC4@UbPW0h@úp#~ŠJ?½¹¾'B?o3§ƒYi½?¯)9£P@I¤µ¬t¾?ŤĚúÝ¿æoû:ža¿ã@Ï_~¿åÐx=~e·¿ãJwB+ɇ¿ÉLáłU°OTHERunk1RXS J164117.0-594647?ïûÇØàñ?2Š†«Ÿ?@àœS1Ô?2Š†«Ÿ?ïî¨î\z»?pSVLŒ»?aW…H´¼?pSVLŒ»?ïóäwIŸ?[ãûR÷<Æ?Yø6®x?[ãûR÷<Æ?ïû±:0c±?) Æ`ýç?A;Ž(*£?) Æ`ýç?ïô`'ï?QICOg?W?¯ –?QICOg?ï­	‹Í†º?›ŽF˜`?"½œþßá«?›ŽF˜`?ïçåàw­?sF}ó_Ûu?hZøí?sF}ó_Ûu?ïëIJTj™?VNèz»"¤?d¶µ|Ú·=?VNèz»"¤AGN4FGL J1642.1-5428e?벲ђÉ
À¸ñ.ñÀ8ãíóŽ¶À;5@qà,@"¸	ò=@÷`¤……æ?ÂApã—êm?ʳ<'è'F?ýÌ–›¸X@cbezÙ?ïÂä¾®&¿½ûå~ŸmC¿á𯕄a#¿éikž´‹¿à
Ýað`¿Æcê
J[ÄOTHERspp3FGL J1645.9-5420SNR G332.5-05.6?ïƞÏ'^Ø?°nzÁ)µ?|°˜y_¸?°nzÁ)µ?ïÕďN?¾`þ˜?uý.#æ?¾`þ˜?î›itQ¥S?›«b҄³?¦Ih»Á'Ï?›«b҄³?ï°@±îF'?m'zÑ®0?ƒïӅGŸ?m'zÑ®0?ï+OœþÜr?™Z¥lÁ?š–ZýÅ?™Z¥lÁ?îâìþèË'?±^º êߜ?¡Ñ0O4‡?±^º êߜ?늁o–ç?©¿…5ï?ÁÕúC¹¤b?©¿…5ï?íóÈ3Wg½?ŸW'†p_?°a¾fü?ŸW'†p_AGN4FGL J1645.1-3323¿ïÃ%(Ùh@ÇäÅøÀ:b/‹ÞÅôÀ;ÇŸïôð@Ñ¢'dì¿@Ayaë­c?ij»¤†]?œ2EfUcN?Üq°œj"X@mF/9?ïìáxU¿Ìp~WÉÀ~¿éšÁÀ	¿Ý¾Ùå9*C¿Ük
…?›¿è\v"œ;OTHERunkAT20G J164516-331816?ïú%{m<L?FKÓõ½òÔ?Gj°Í?FKÓõ½òÔ?ïÚ÷"¡?\¬´—Œz?rø"/ír?\¬´—Œz?ïÖ´QÞÎ?x'ªë½/ ?t¥ôl^-?x'ªë½/ ?ïøíZÈÔ?36#HF¥?LJ"ú@m?36#HF¥?ïÜU0^·?x&@¿ó?qÕgÝS<œ?x&@¿ó?î·
|Êo¿?²Zðt`"?¤X1¡6?²Zðt`"?ï^e‰zEI?'	áÐöð:?"3NזŽÔ?'	áÐöð:?ïÔâªJ'?g¿&f\-?uŽý}"?g¿&f\-AGN4FGL J1645.8-4533c?î#ïlp&뿧.€_ЎèÀ7Г¨¾Ð‹À9zc'ŸÐ@ê¶W?ö@DV;u÷Ô?À`"•N?ÐÈá°´"@àÀ_?úål8br?ìVP%"õ¿Þæ[L
¿åƒÚ_Ý`C¿éÉÇÄ¿ì/_i#¿è™¢¾[oèOTHERunk4U 1642-45?ÌbôEP…î?Ï&pH"¿¯?èçBî«Þ"?Ï&pH"¿¯?ɂq¡œ·?Ád$[˜ÆÐ?éŸ|c—˜Ò?Ád$[˜ÆÐ?Öå20¡)þ?µÓI¦ð¢È?äfç¯k?µÓI¦ð¢È?Å¿~\úN?«	Þûy*?ê xèÁl?«	Þûy*?¯Úûé¹ÐB?Äè¿O>_??îPA-i<?Äè¿O>_??"̵G¿À?šô}"½³?ïašWbE"?šô}"½³?°ê'Š@"? Âáúڝ?í⯿·î? Âáúڝ?hI'æÚÏ?_ZœÈQ?ïç¶ØD=?_ZœÈQ$PSR4FGL J1647.2-0154¿ï÷K²·Î@:T;ÄÒ,ˆÀ;üè‹+À=»	h_@ wɉv`Ú?üó÷é±	"?ؕ";ᭅ?ïû³ŸÕý@ÏE™›@¥"ºÔõ¿ïÿÿ" 5•?ïÿò> w?£	1à€fu¿Â"ÏÅЄ<¿î/é¿ïÿ}e†mOTHERglcNGC 6218?éò»£§?ÆÇ?ܱ=È?È5qcçÓ?ÆÇ?ܱ=È?â³ñ÷©šC?Ð)d)— h?ژ¬Ë{?Ð)d)— h?êeçÅ'ï?«;Åq¥?Æh`ëÁôE?«;Åq¥?Ü©^¦²Ž?µ1=_˜Ñ?á«P¬¦ø¹?µ1=_˜Ñ?áÕé¸Y¼ú?ÍZʀ0*Ú?ÜT,L†
?ÍZʀ0*Ú?Ðì1½£uL?Ñ	'ä&cJ?ç‰ç!.EZ?Ñ	'ä&cJ?æ—"¡É›?·D¬úb?ÒѺ¼mÈÊ?·D¬úb?ÂPÝ»åýS?²ÁÐ;²­?ëkȑ€«?²ÁÐ;²­MIXED4FGL J1700.1-4013c?ï™ønçu?ôãŽ)ùΎÀ9+©EGÍÀ:´Zøt"@Ä=®·8@@›ùÆ*?Ëq†Àyt?àc!m8¿@âÊÿm3	?ÿEÚdåÝÀ?ïÿô!O…ú?Í°:ˆ¥Ö¿àý)áпö¿ë.ª¢ÖY>¿ébߓxî(¿Ýs—ºñƒOTHERunk3FGL J1700.4-4019cNVSS J165941-401121?áâ,Ø®"?ÒÈ.­gÄ?Ü;¦OÆ¢ø?ÒÈ.­gÄ?ؤ Ãfi
?ÊÄT¬bþ?ã­ïžLËy?ÊÄT¬bþ?å+ÛÊ®Å?³¿ÞËf–?Õ¨Hxê¢v?³¿ÞËf–?áìæ¦ì?±&|̗Å?ÝØ&3è²(?±&|̗Å?È&#©òq?ÅXürp>?éöw?ƒd?ÅXürp>? {¥bc?¬3OjyÛ?îþÈE壚?¬3OjyÛ?É»7¦p©?²ë`EA?é';2cÖ?²ë`EA?¤È2D†þÉ?'³XyÂ"u?î³|Û·?'³XyÂ"u,MIXED4FGL J1701.0-2617?°W0Mn«@#Q2rC{À:zÝì¯ÁÀ;æiŸ
w@o=O–Á@Ö3Îc¥Â?Äóöû‰#?Ä
‰w¹?üv[ÁǶ
@V^Ä0›ÿ?ï	GÂ6pÕ¿â
Fªß<¿èݘ—;ˆ¿Ö&ˆ_µr=¿é"^úŒN¿çAÀ>ÉêOTHERunkPKS 1657-261?ïí~û€
õ?k$š(f¥?b¹®{?k$š(f¥?ï½&¿(í?‡²Þ»Áõt?€¹v\<fÅ?‡²Þ»Áõt?ïÍ9<?T?xw*<Â8¬?ycaåÕ\À?xw*<Â8¬?ïØùÏAúª?TbVn&
?sƒyϞì?TbVn&
?異û±Ök?Š° bE0?†—AÉ=?Š° bE0?íývêSW?¸Kt¶âßò?°Fõ—M?¸Kt¶âßò?îßèŽ?¤ËV\|•?®'Ä¢à)?¤ËV\|•?ï{ÓQn?…"Ó«Ô?žp›üþÌW?…"Ó«ÔAGN4FGL J1701.2-3006¿Ã+]¼HÆ@Jì$·oÀ8©2ëƍÀ;"'>E@V.?ÿà2Š–ÇW?°1§—ß]?؅»@]h;@&ÇH!Äv?ü^ÖDoƌ?ïþFA'×5¿ÓP&žzT¿ÝBã_5o£¿ä''wcå¿îɨ G³ž¿ïÿuᮆ;OTHERglc3FGL J1701.2-3006M 62?Sv=¯p?Rÿ÷ͦ™?ïöDá*ï?Rÿ÷ͦ™?°¼¯{Ä`?¬†Ë1}a¼?íèjƒÊ"?¬†Ë1}a¼? ›e€ö%?–Hþ·Û—ú?îÿI~µN?–Hþ·Û—ú?A[©d?r¤Å

??ïÀý}¼Þ?r¤Å

??j4ƒ™jÞ:?où*äD?ïåË|HX'?où*äD?ƒ+î(谜?‡
ªÐd6?ï³PGsº•?‡
ªÐd6?‡"Ø-°?y՘{
?ï£wÌÈΙ?y՘{
?œ´µR'ý?°ºI¡>?ïÿcŠ"Œ?°ºI¡>PSR4FGL J1704.1-4140?å<Š+ßÏ*¿Æ᳤1ÎÀ8à8¦À:æ5SŸ@ lZ$c·Š@<å;X›£@ÏÓ¥."R?à/SàQäÏ@îÀrKv÷?ý'Êß·¶?ïöÉ™"{¿ãïD[y£Z¿âµj¿'{¿âŸp"§Êµ¿é¹ñÞ&Ò¿ïÿ2z¦KOTHERsppSNR G344.7-00.1?Ö>'>C˜Â?Ôìz¢2š\?äàì`Þ3Ÿ?Ôìz¢2š\?åmÙ+¢<£?ÒbG¿"¬?Õ$M¨»†º?ÒbG¿"¬?ۄƒˆò=±?µƒ"Ñ?á?â=¾;†á(?µƒ"Ñ?á?å|¶E»Ò?Á Õ‡]W?Õ"tˆà[?Á Õ‡]W?´ª*Çýû±?Â6oÜ9…?íjº§
þú?Â6oÜ9…?ÐÃÄwyð?Ñè:?Û¦ô?çžpÄC?Ñè:?Û¦ô?Ö ¼"°"?·•rԚ?䯡õ?·•rԚ?¼¹ê"?¼s׬éqb?ì}¨ÞlB°?¼s׬éqbMIXED4FGL J1705.7-4124?ìäۖ$6¿ÑA…±ZÀ8q=†ÅÀ:ÅÒ݈@NQŒÂ@]lÝxì{?ÇñPå ®6?ˤK¤C@Ç@ˆ…ZGt3?û½-Dܨã?ï­tw¡!M¿Íœñ½Ç÷%¿åÈ
L4¿å@@aïß!¿èê'Wގ¿ïù+àŠðOTHERsnr3FGL J1705.5-4128cSNR G344.7-00.1?áêq'-X?ԙbîrõý?Ýô+Û¥O?ԙbîrõý?â‰À+ºÕ?ÎƧµ¢Iþ?Ú쨊Uâ?ÎƧµ¢Iþ?ÚFvtþ/?·ãßDý¹?âÜÄúE€é?·ãßDý¹?ãaÅGÐק?´_?¹½÷(?Ù<up^P²?´_?¹½÷(?ɑքÜs?͵ü\C£?雸J^Èã?͵ü\C£?¼dšaÞd?èÄô?ìsl½SÄ4?èÄô?ϸ}NN0?´AÆ$s0?è:'à¬lt?´AÆ$s0?°ŽEPÌ¥? ƒ¥–?íî7V6 +? ƒ¥–MIXED4FGL J1708.6-4312?ƒ'2¢&¡y¿ü4 HtãØÀ9¥tæXÀ;æñ;A@'2]jÔ@N¿ö$µ?ÍI>7s3Ô?Þ8ÞîãM@YДØ@°{/Ì ?îÅ&æÖ«¿ÚWq S²…¿àºëÄØí¿ãÂ!­Ï±"¿ïVNád‰l¿ïT?‡ÕK÷OTHERunk1RXS J170848.0-431418?Ýl1Ó.?Ë?¯Dž?áIçq}é?Ë?¯Dž?åkð"6ê?Ç¢¿óuƒ?Õ(Ìג+?Ç¢¿óuƒ?ä%‰?³«ú^‡H)?×ѵÐíÿß?³«ú^‡H)?èÍw"=^R?§xÕÆô0?ÌÊ!ï
†¹?§xÕÆô0?ÂWé֝Ûô?»igUWS?ëjŠX‰?»igUWS?ÀÞ‡Ú2?ÃРÜw?ëÈzž	sz?ÃРÜw?ÂQ<§?®¼`0%ér?ë|ë¿ðà?®¼`0%ér?È°ûÄö®a?©Ó·êÀè8?éÓÁÂTh?©Ó·êÀè8MIXED4FGL J1710.9-5247¿î`{K-ƒyÀï•·UlÀ9þ¹®âÖúÀ;'óá
Ì@N0Üêù@ÞÏŒ0û?ϝ^ mÿ?ÖÔìԍ@ð¨ß‡ºt?ó?ƒ3є?ïÇ:"ÀÅ?Øá=\¬Ô4¿å0†yÇ¿í8⟜é¿ïÿú Âî'?ïÿjÿR[OTHERunk1RXS J171043.7-530019?î£JªÉà?ÀÑU‰?¥ËUR'«?ÀÑU‰?æ´^ÜÍe?Ë(jWa»²?җCöFe7?Ë(jWa»²?콌uø2_?¢B!ˆqñ7?ºœP>m	?¢B!ˆqñ7?èaem?±x¼û£™?ÏëæzjKÆ?±x¼û£™?ê¡Èè<?Àõ8"^|–?Åxߘ_Ž?Àõ8"^|–?ÂBCˆ?È?®‰ë§?ë|ïo9Ù?È?®‰ë§?ã²zÙŽ\?µ1ˆ$'†?؛
MòãH?µ1ˆ$'†?¼+<jz®X?«Làçãˆä?ìz˜r°ª5?«LàçãˆäMIXED4FGL J1711.6-3407?ïo+A]@	"Äv£ËÀ9Ÿ6'Ú9À;$É:q@vŽôÏö"@¦NÜ%´?É;Û7ôŽ?ÉxրÂ-@¯~Þ,q@ö™ŸxÖ«?ìÚʆ¡oQ?îÝIúÑÿãÜÀ•†åb¿è`´á¼©¿é/Q/|¿á׊`@²xOTHERunkNVSS J171151-340701?ïhE*Eg­?"@?ŽŸæ?'÷Z²+ h?"@?ŽŸæ?í1g&æÚÑ?µQ)
IáÊ?¶tÆÉ7ö?µQ)
IáÊ?î;Ýô'cš?›È,M<©?¬B µ!ø]?›È,M<©?í¬À):8?–j~)úÅñ?²™þ¶ð:½?–j~)úÅñ?æú¡È™Ñ?Æ,¸Ù$¨?Ò
¼änÌ^?Æ,¸Ù$¨?á-²rOö?Ñ'Œø\®¾?ݤ›`ø?Ñ'Œø\®¾?ᘺœ§Ä?»NÑ<{¹è?ÜΊƱÄx?»NÑ<{¹è?àë[roÅ?»¥˜¡.A?Þ)Iõ u?»¥˜¡.A	AGN4FGL J1712.5-4642¿å^kò'¶dÀ'^!ôGÀ9˜ð¹À;)Y•Œ@°ìaŒ@ƒxÅä?È¥©GÎ÷?Ü'q~Gƒ¢@óg†!Ñ@¢"¾"y¿×|z"«uå¿å}IÔ+¿çá~o¿é€kà£Ä@¿î""¼ÃjM¿íú¾z$OTHERsppSNR G343.0-06.0?åXñÎ~g?È«ŸÎä?ÕNcõ3?È«ŸÎä?ã\7ƒ¢?ͬJqúT?ÙG'Öùî»?ͬJqúT?èÚ¡'Ç3?­Ùns_¤ÿ?̕{`ã3…?­Ùns_¤ÿ?çÛÈA:?®Eý‡`Ï?ÐHo}ï͋?®Eý‡`Ï?ِÖÓrª?Ê=˜k5?ã7"–Fö+?Ê=˜k5?À
qFƒ
ü?Æ9S?ºw'?ëü£®_=A?Æ9S?ºw'?Óó$¿ï?´îÅ'™|?ær†m u	?´îÅ'™|?²W³øÃà:?£ODÁèýŒ?íµ	€Ì?£ODÁèýŒMIXED4FGL J1713.5-3945e¿ÈÑ@"²¿¿Þ@zcÉSÀ7aÿ¨Â,À:fpÍÈu@";@1ôD?ùµ *­R´?¥#Rj†¾?°Ôñ‰o«@aw]?÷Ž²Jj‡]?ﶘ]Ywk¿åہ›v¿ÐŸv¼Ï)¿Ñ?áAxñ¿×Ś^:á¿Ô…·eOTHERSNR3FGL J1713.5-3945eRX J1713.7-3946?ãLØç&?ÓíJ.?ÙÍfOÀ1´?ÓíJ.?êgi!̕?È!
);ì?Æb[»xÍ­?È!
);ì?嗡Êô
6?´ÿˆV%Pœ?Ôмjå"?´ÿˆV%Pœ?ç‹%¯ßM¥?º¿õ	='?Ðé´ Adµ?º¿õ	='?ç]H)Âá?Ìh²ªü\K?ÑEná¬z>?Ìh²ªü\K?ß[L&Ÿ& ?ÓW5>ƒÑå?àRYì°lð?ÓW5>ƒÑå?è³_t?ÿ?·Ý¹ ãô]?Í2'/í?·Ý¹ ãô]?Õ¤)®©?ÂKŠS;Í?å-ðë(ò+?ÂKŠS;ÍMIXED4FGL J1714.1-3811¿ï÷&¡™1.?×5Œ	À8ÃÌõçxJÀ:ºæç*F%@"/ÊF_µÈ?ÿ %9um?»"Ci6Or?ªé^ºS+?ñ+E"ˆ¡@}:«w'‰¿£™1"́þ?ì¦a
¶ø¿Ðþ<[zû¿ÝNjܗÆ¿ß/Ÿ•\7¿ÝR€*‡¾OTHERsnrSNR G348.7+00.3?ï³ÉöŸ?¡Ïv›ðY?ƒ
¿—ÃHD?¡Ïv›ðY?ï{ÏN‡L?¡î{?³Á…?†0Î;þ?¡î{?³Á…?ì; •j?¬¬É|TG'?¿¾"ûW¤­?¬¬É|TG'?ï½N¡ðø?ŽMc<
Âù?ŸÈV/1|í?ŽMc<
Âù?ïœ=7îÚ?ŸïG|ê'?œ,xSÚºÐ?ŸïG|ê'?íœݖYÚ?½1û5üø?³áqJ/?½1û5üø?ìÁÆú$ô¬?­Û"^øü?¹ñÈ.ØZ ?­Û"^øü?ëvUŒc?².>inä?Â&«âÎr?².>inäAGN4FGL J1714.2-2928¿æȜ\Ó¦Â@¥w–9'ÉÀ:Lp–À;"7À`­À@"ò}
—´@
ˆ~¿"À?Ìéÿb¡4î?Ù
°Â«
Û@—'YY7ª@µ2Ò:J¿ï?Wc"$?ïÿ×á¨Ññ¿ä¸¯©¦W¿âá4bÞª¿îa*ÝyBa¿ïþ]~
qôOTHERglcNGC 6304?îYöÞ?±v/Ú~µ>?¨ºc*× ?±v/Ú~µ>?ìQ·5‹Ó?ºÞ/u¹jš?½sFS¡h?ºÞ/u¹jš?ì6ߝxÃ?¤DÙá£Â"?¾Iü9ç?¤DÙá£Â"?înzºŽå?ŒûXI™ÜH?§éPçu±?ŒûXI™ÜH?êóhá_?€¸±%Á?Ä2]Àz"?€¸±%Á?Ýß=ã:wu?ъðE›&?áabÄE?ъðE›&?âEþ—Ó¤`?¸àûs	3?ÛtÐX·@?¸àûs	3?âÇ{ë™ý©?¾!䐧œ?Úq(Ì®?¾!䐧œMIXED4FGL J1715.3-3832¿ïp3X¿V9¿ªl^Íë±À8ƒ~Ù#ó$À9¤*ëf@£#âqŽ@O	zÓõ?Òµf~ºC?Öa¨üãëÍ@!µÇ͉‹@G+ù4ä¿Â?$ÃÍÕ?翞æàtI¿å^*Ýúº¿èYP¤«›¿ë¡›%ŠÔ¿ïê­R´ûOTHERunk1RXS J171538.1-383531?â
£%Î4›?ÔŪ3š·&?Ûê¹´c–Ë?ÔŪ3š·&?àÑÕ§´0ì?ÐJ%kR"?Þ\T°—ž(?ÐJ%kR"?ÝðJ~1ø?¶£Õ'|U?áÚÀçw"?¶£Õ'|U?åÝüMÕ=?·«HSçïÏ?ÔDdUó…?·«HSçïÏ?ܱgµµË?ÔÁ`Ä?á§L%%1?ÔÁ`Ä?¸ßm‡$?Â4hŒDq?ìä\+­‹?Â4hŒDq?ÅfUzììc?±°`žEé?ê¦j¡DÄç?±°`žEé?®gQzN?¤¦€Ìq©??¤¦€Ìq©MIXED4FGL J1715.8-4549¿ïA£6YÀdÜ"«%³À:oÅåÀ;o§ÿê9@ZÉ!œ‡á@^ne8hý?ÓÒo##p?ç%  ß^@u‡CUÀ&?ÿgþÏSd×?ïό/MËe¿×ÛÙ°
g¿×ED'»Ü¿êE€½ªšô¿êm[}Ë¿ê…M²:zOOTHERsppSNR G343.0-06.0?Üï§	f'Ÿ?ÎNªÁùÎÒ?áˆ,{Lì1?ÎNªÁùÎÒ?ßþHÖ?˓@ÍX@'?à۔ˆ/0?˓@ÍX@'?åóŸöf4y?°Ë°»³Å¡?ÔÀ3—?°Ë°»³Å¡?ã;má§G?°‹¦d¶Á{?Ùى$<±r?°‹¦d¶Á{?¬gxPœñ*?±âsR2&ï?î9ˆ{l=?±âsR2&ï?µÎå¼t?Àç'`Ý\ß?íF#Hb"?Àç'`Ý\ß?ÃÃyº´¤ë?­ðö]š?ë!'RÖÅ?­ðö]š?²mhƒå?žÈ%¾ÝI?í½2R¸‰Ÿ?žÈ%¾ÝIMIXED4FGL J1716.7-2808?âXv$ÁÎ@ú&€IRÀ9M'¿°"˜À;'íû½ñ@­ç"^@Ìã"y§Œ?»ÙÁÎ7?×FW}?pÙ@ªTà,%"@ÜðJUd?íay,;È-¿ßÏÔ¿	•«¿ÜYB'uê¿âÿO™›G¿î3eˆ¿ïòüÂ÷ÆOTHERglc3FGL J1716.6-2812NGC 6316?É|@²U[?Ì´‡"µ?é úïÓj©?Ì´‡"µ?ÕÌc­›Ñz?ÉFI¡?åÎ)2C?ÉFI¡?ÑFœôUë?³vb%"¶î?ç\±…¸U
?³vb%"¶î?æKä%óžb?®%{vؕ?Óh7´Ã=?®%{vؕ?³Cg™"m—?Ä+\`¢`?헓À5m?Ä+\`¢`? N6áV?¨')þjÏc?îû,¹¾Ê?¨')þjÏc?º4T«—¸?­BºÉ@Ûz?ì¹nUj	?­BºÉ@Ûz?À7ÓÅ©0Õ?¢Ëáy)?ëò•³Ë?¢Ëáy)MIXED4FGL J1716.8+4310?ç¦}"¼@Au¥ 8LÀ:¿,;È-+À<€g€AÙ¿@l[…íõ@¥Ÿ<pÊ?Ò Š#¯Ý~?àȶd«{@¤ò®å¨@ñ`°D
¿ìõ¶ÀÆÚ¿Ý c¸6<Ó¿äBej½ãü¿æXh¬'Ãâ¿ïÿ½OG"?ìf³ÞiW]OTHERglcNGC 6341?ïÞJ1Ã?sϝ\}Í?pÚýxL~?sϝ\}Í?ï†eAÎ+?—º0¦æþ?Žf¯'&Dê?—º0¦æþ?î^þ[N?•¸²¹mx?ª"?•¸²¹mx?îö˜6(lA?ˆãɧ`˜? –|™-¸ö?ˆãɧ`˜?ïäyÂå?¡žœYZP?žã|¦Ûd?¡žœYZP?êoîpǤ€?È'D@æhï?Æ@F<án?È'D@æhï?êOXß®ë?±G;U
?ÆœDR?±G;U
?ç¯â陷!?¸Ùu
"Ö?Р:,̑¿?¸Ùu
"ÖAGN4FGL J1718.0-3726¿á#îaœýý?ÄÅąU"ÝÀ7}5¨Xy>À:*ôàM/@ Œáºö·@Ϊ¦1?©šÂÓ=™?¯J+Ú#@¶w¦)ÊÕ?ûѺyãò?îÀ]ÔÏ¿Ø`Sý®(¿ÞÛ¦d-Q¿ãOl-Îo¿åGÞeü^¿ãÿíPÐÓOTHERsnr3FGL J1718.0-3726SNR G349.7+00.2?à,›5ó?Ó{ЋHH?ßòå¦É"?Ó{ЋHH?éysH÷ë‰?É
ýu>Ø?Ê2Ü QÚ?É
ýu>Ø?âØ}7%?¸iRS.Ý*?ÚO÷Å¶?¸iRS.Ý*?äíµªhÁ,?½dUCm+ì?Ö$"«.}¨?½dUCm+ì?Øç{÷ßå?҈M?ãŒB|?҈M?Û£-
¡ œ?Òµ0Qi?â.iy//²?Òµ0Qi?å`Ō*Š?¾¸qÜfH?Õ>tçªëô?¾¸qÜfH?ÅÔ:Æ5À?·£,x*Ÿ?êŠñNrü?·£,x*ŸMIXED4FGL J1718.3-4445¿Ì'–NFÆÀ]'@.Ä9À9°"6[àÀ:áJß!c'@ …úUq!@ºizíÜè?Ñ3éܨ#?¿«ó¹J¹ã?÷rï
å?ÿ_Ñâ5iÄ¿ÒC¨ý?ï!ÿ¯"B¿ç%ƒ—×ø¿ãV;`~Dÿ¿ëÑ4Û©ßb¿ÛŽã»{ÂOTHERsppSNR G343.0-06.0?濫̸k?'%üCÕ9?†×LþA-?'%üCÕ9?îj¨ç"!ý?°5²it8?©Uq‰u®/?°5²it8?ìp†cÃ2?¨Cõ·ÍmN?¼{ÌáçÞn?¨Cõ·ÍmN?îtt°ú?'gÈà/àU?¨¸·Ž"f?'gÈà/àU?ë¼É ½1F?¿$Í:—ä?ÁÛ}:é?¿$Í:—ä?ç·P‡4šÅ?Ñð8•Pg?Б^ñ–Êv?Ñð8•Pg?èBXVG#D?µŽÄ¥?ã?Îöž¦ãrð?µŽÄ¥?ã?á˽'z?ÁEß%rˆç?Ýòh…Øû?ÁEß%rˆçAGN4FGL J1719.2-2943¿×1ï¨ç6Ó@}¿Î·ˆ˜À9Ú¨ÎÀÂÓÀ;(ÇAr'@ !f'jþÒ@¥BDH.?ÂXIؑ&.?¥Ä`A´*j?Ø»›!."þ?ö"±ší+½¿î¸G¿²2?麗*¿ÂypÚ2»ê¿æhÓ]à…ç¿êèûlˆÍ?кѢŸ|³OTHERsppSNR G356.2+04.5?ïœN÷x¶º?'gþ5pM?ˆìBƒ}™?'gþ5pM?ïeÊ<Ø+?§î®ŠF´R?žsF¿D2'?§î®ŠF´R?í¿LS8ë? Ò(Éº"?²g0E*? Ò(Éº"?ïÌêB©?‰äYf3?œ¦}"oxÏ?‰äYf3?íõ\"ÝJ§?¯žéTÛ?°Uañ'Ç?¯žéTÛ?é…‰OÓ?Í'eaPs?ÉëõÚÀ³í?Í'eaPs?ëα]§óF?©CBü¨'i?ÀÅ:‰`2è?©CBü¨'i?襩?Ýn8?º%±jp·"?Íi[ŠG?º%±jp·"AGN4FGL J1719.5-3858c¿ïì;gŠ'â¿îýÕôéLÀ96^q¥^ÊÀ:‹™¯i·@€‹Ò† @Õë#Ïèá?Í:†ä‹/t?ÓÄ7Kæ@tËáëB?üû]y,畿ïÔY=ÞÝÆ?ïߘa5O¿âÀŸAú m¿êD
û¿ïú}¢Ã¿în¸å;rOTHERunkNVSS J172006-385734?çέjºf¡?Ð6''p2÷?Ðb¥*‹2½?Ð6''p2÷?ß=ˆÚ2a?Í£_O4µX?àa;'¹fÐ?Í£_O4µX?ãæg~`r?¶$‰rìû?Ø31Ó??¶$‰rìû?äp†ýNŽ?´
zR[¶?×òbâÆ?´
zR[¶?Õ&¹A'ã?Î¤Bô?ål£_s¶?Î¤Bô?´s<Y¬×?¿|#g
U?íq˜t¼¦ ?¿|#g
U?Щí¾x»?·lÀ~:¢?çÀ+	 ã?·lÀ~:¢?®ß¦œ¡Ö?¡ªt¿6å"?î–léb?¡ªt¿6å"=MIXED4FGL J1719.7-4500¿ÒM™ƒý® ÀÃkL4"À9°üQõ–À;¥5¯v@H·"ª—C@Ók'/É?ÎÙ6´Þ?Å°"UÕJ?þ*Óé À@#T²^âd¿ËP§!íeŸ?ïüFlÊ¿è2æ§ieõ¿áȬar`Æ¿êv?A´U]¿ïՓWPOTHERsppSNR G343.0-06.0?ï7܃V¿³?¥yÀZTˆŽ?™o"p;¦?¥yÀZTˆŽ?îÔuÒXìš?¦G4ÿQ‰?¢¸¢Ýë\?¦G4ÿQ‰?í×üc[?¡ˆæœkUð?±@:¦ñ¦?¡ˆæœkUð?îÒuuDr?‡-ʎe%L?¢Ø¨©%)?‡-ʎe%L?è÷mÐ&ž?Ä¥q/(rÌ?Ì"H¿·e‡?Ä¥q/(rÌ?éë9õD:?ËÊuš¤S?ÉøS*ï?ËÊuš¤S?å/R†"5/?¸"°çu?Õ¡Zòٕ¢?¸"°çu?åM=Ëñ
Q?»`¿>?Õe"hå]?»`¿>AGN4FGL J1720.2-4757¿Ü"jÈÏ_ÀÀÓI¾óÀ:'˜Ë=À;K§ågÎ@¤àDMâ·@¡/ÅÀi?Þ³ÞY<1?âéà¾ò·@	å'^éšc@ۚÅ都?îÁr'¿ãF¦ã.8"¿êí¦â'Q¿è"s?ã­¿î±CD"o¿ï¤rØœOTHERsppSNR G343.0-06.0?ì?f[Ãd?Â8`Œ»Bi?¾Í!äßÇ?Â8`Œ»Bi?çʒl3&?Çnu5ƒ'è?ÐjÛý'™³?Çnu5ƒ'è?ëáÖ4]2i?§oNDñ˜?Àx§.‹6]?§oNDñ˜?éžxV†}?©y"uˆ³¼?Ɇ¥æÁ?©y"uˆ³¼?âLgv°¹?ÒÛOµ'1?Ûg1ÀžŽ?ÒÛOµ'1?ÈÌl
?Ì|išö?éÌäø<½ ?Ì|išö?àæÄÒy×T?ºƒ–užé?Þ2v[QX?ºƒ–užé?¾V"4¥¤?­.vlé™?ì<Õ-™kK?­.vlé™MIXED4FGL J1720.6-3706?ƒ³(xÒÌ¿°¸XÌtã,À8§?LF)°À:1²þÅm]@>w|ŽEþ@S½Ö.u?ǚÕChài?Ø ê@%@6Vîú??ô–óT Å?énÑnòý¿Ü.®¿²‰¿á½I6ª¶ø¿èÚå>]³º¿ïÿðEwÙU?ØddIU´OTHERunk1FGL J1720.7-3707c1RXS J172051.9-371033?ѹ|Þ ?҄î4Y+ž?ç#Aùþð?҄î4Y+ž?ÉkWæÙ?Â*˜ÿY«²?é¥*;½ÆJ?Â*˜ÿY«²?Ù©:˜Ï'?·Ý¤ðS©d?ãp«b³˜7?·Ý¤ðS©d?ÆÖRBÔ!;?¬>e«Ö]?êJkoJ÷±?¬>e«Ö]?©T	ˆ
+í?¹¢økk"?îj¿gšª!?¹¢økk"?'ö…¹Û
?™Î¼#!ç2?ïhKÒL¤°?™Î¼#!ç2?­‰ò¤ÑÞ?²‹FßQ?î'`Õéè"?²‹FßQ?gËä/˜´?[Oúïíߧ?ïè4æez?[OúïíߧPSR4FGL J1720.6-5144?݁¦~À ¹y[5°¼À:¦úX÷À<"hê¥$è@ ²šl'p‡?ý	¨ÛUüŒ?ÐŒ¢:R?ÐÜ¡'N?ÿàjْ­í?ÿøwWû>¥¿Ý¼âÉä:¿ïÿÍ?¹Ss?ïÿþøþ"¿ÂÜËG'	¿ç+ÔÏЍL¿å»¶ŸŽÑOTHERunk1RXS J172032.0-514414?ïöÜèù©$?lçŽÚàí?RF.­¸`?lçŽÚàí?ïÉl¦O??ˆÆ>¢®êY?{I¬ä%Œ2?ˆÆ>¢®êY?ïµÛ š?€ö¯.ŒF~?'‰?¾Ê6?€ö¯.ŒF~?ðxx?sÌóz¹¬?‡׬Íõ?sÌóz¹¬?ïîrÑtã?^Ž\Ùݜø?aîœ·?^Ž\Ùݜø?îüƒÁH¾?²˜ƒÃu? ?çÍ%?²˜ƒÃu?ï$í«r<¼?•_u·Š?›bJ•(|?•_u·Š?î¾h}dQ0?™ùZIÏ?¤x(?™ùZIÏAGN4FGL J1720.7-4629¿ï£='¹éÀºÆü©3kÀ9«;_QŸ/À;蚈¬â@,Z¢7øÀ@
=f?Ò&Mà]£?Ú
™¶õÊó@ýÌI?ü…jpUÊ¿àŸÖ"Ì«??ïø m]Ñl¿ë<7ž|ØC¿ïg6¥®zÒ¿ï¦J'Qž?'rs\e~OTHERsppSNR G343.0-06.0?ï˹èL7Å?…]´r*B]?z#Ðõ!¿?…]´r*B]?èÆ#lZ‹?ÆTN¶Ç?ÌçrN•Ô?ÆTN¶Ç?옜¬7p?£mt›µ?»?ëžD'?£mt›µ?ë6âú­ý÷?¥hd ò ?Ã$tH$?¥hd ò ?î³(P×?®¸]ör'?¤Ízõÿ
?®¸]ör'?ȓ¡l´x?ˀ…¡j€?éÛ½$Òâ?ˀ…¡j€?ã,ÈrÊø·?¶Yp.>˜?Ù¦oj'?¶Yp.>˜?Æß#«D¬?²e
­Gn?êzH7.Õ?²e
­GnMIXED4FGL J1721.7-4709¿î‰Gj*sÐÀºeÏg±ÀÀ:Ɨÿe¦À;œèÔjP@£©blD@¥ýfȌ?Í喝:ã×?Ò@$]Wt@,^b‹æS?þ-
gbé?åùæuë>¨?×|Š_iòã?ìÁ֙Õ(¼¿æ˱ÿÁ쟿ޒñì7Ì¿ïþŸã_¶IOTHERsppSNR G343.0-06.0?ïÄ´Ãt<?€•%.^­?}¥žIQŽ°?€•%.^­?ï&ÈJÃ?§Z.n¯3?›&üoÜï ?§Z.n¯3?Õ2n_?–kù˜õ¿;?¦2¬Ù?–kù˜õ¿;?¿?'°‡l§ec?§Ž•°[?'°‡l§ec?VDÁa?¡«¦wÊþ?¤¶Ê˜DMð?¡«¦wÊþ?유£_QZ?ÃB­É
?»úåu,?ÃB­É
?êzñZ~Y?®"IUo?Æ:–›?®"IUo?ê"ÆU†¼•?µƒ$¸9í?Å°æ©å
®?µƒ$¸9íAGN4FGL J1722.6-4529¿Ùl3¼½W†À…³ž'ÔÀ9¯Ëú>õßÀ;²Lþ
@ÝS­§@ì``'çÏ?À9yþ§?ÔØVB×Àò@'j¡^‰ù@kn|Šj'?ïµïpeé¿ä±¢Íõ¿ß
J 4¨Ô¿ã‡#uP5¿ë©ÿBjß¿ïúêû‹ýOTHERspp3FGL J1722.9-4529SNR G343.0-06.0?ài!&ô¿
?Ê'Jc?ß-½²æ?Ê'Jc?ì¢
Æèd?·Í­kŠG?ºï'È¿Ìß?·Í­kŠG?ä*F+ñ?´'Ûdj7×?׫ÅsŨ?´'Ûdj7×?í¨xÁÕo?>lòí?²¼9ñW4‰?>lòí?ÀÁëáÿ©?º²—Azž­?ë؏…€?º²—Azž­?Ú²Õ""?όÃcRÆÞ?⦕xwµï?όÃcRÆÞ?Âm[k>E?±cîP7øU?ëd©%0n»?±cîP7øU?ár›áÐó?±y삯#B?ÝÈ<^ÿ?±y삯#BMIXED4FGL J1725.1-3408?øΊbð?ë2~žºÀ8ß\Q9®wÀ:I‹N};•@N.4ñ¤H@îu5¬?ÉNÚX¦Š?¸Í®ôõ‹?óü8Dêëœ?ü§5Ù«­m?ãØ'>2j¶¿Ú»k{y"¿çRª&¯—2¿åjþ¦Ž ¿ì¶ ¸Ý,¿Ø/EâOTHERunkNVSS J172445-341032?ç+0­¢v?и'X1Å?Ñ©ŸÔ¤»?и'X1Å?îE-8ÈH"?°©X _nk?«­,tW^Ä?°©X _nk?äÿÝ°r­?·"«œ'?ÖEğ§?·"«œ'?î,`å·Ä?"éY"S±?­9ñ¨ÏAœ?"éY"S±?â¢17?Ñ÷Z"Ëÿ?Ú»ÁÕϑ?Ñ÷Z"Ëÿ?æѪñÊw?ÐøxÜ#›ª?Óú\ªk?ÐøxÜ#›ª?åT犵~?¹è¢3y²§?ÕV0ê"Å?¹è¢3y²§?àË»ƒŠtÊ?½WÉ;Y·?Þhˆøëm?½WÉ;Y·AGN4FGL J1726.0-2843?îÝ(Έí@
çTm?žÀ9ö·ü[/ÑÀ;Mx2@Äì@ Óc®ün@7‹7GN?Åa°ÊÓù?…³sy8>û?ÆZgª‰+?ü{Ã	ÕkØ?ïNj׆¿âÁž€‰'\¿ç	ýڶſåf:âT¿Ö¯šâÄÜ¿ãyÔ½\OTHERspp3FGL J1725.1-2832SNR G358.0+03.8?ïûž!qGt?A‡îi€Y?A‡z|Môš?A‡îi€Y?ïµ'›ò?"ÍŠé¦Âå?'¾Ûu™£—?"ÍŠé¦Âå?ï¯n,…€?€(o?êÛ?"$}ê7Õþ?€(o?êÛ?ïâ2³=c?Vr­Áùšð?mÍM¾Ü½?Vr­Áùšð?ïøã
ü³D?V!$áãi¯?LsÕ0æ²?V!$áãi¯?íï`²¿§Ã?º2芘u?°"újÞ¨ê?º2芘u?îçVÐ5%ë?˜‡ž8r‰Ì?¡Š'ûѺK?˜‡ž8r‰Ì?ï
±xªØÿ?',hîÊÜ.?žIÐå}v7?',hîÊÜ.AGN4FGL J1727.0-3835¿Þý6¡~¿ÿóÐFÕÀ9á¿uÌ4÷À;ác\ƪ@ëE	¬§@a/	ØÆÖ?ØY<k?éÇE8ï4×@
ÜT^üå™@'Ö†ßÙ¿ÂXG"©¿Ùn<‰J"¿åî'Z·Ü{¿î‰¢«'¿Ô×Q?ãšÅ¿ïÿs³VBOTHERsppSNR G350.0-02.0?­ rã? Ÿ]*ŒøJ?—"›RãD? Ÿ]*ŒøJ?ï+®ßY ?¤äà°Rša?šŸÊíb?¤äà°Rša?ìuguH?¦·é企?¼TÄWEÀ?¦·é企?ï´
ѕ3ƒ?pQç º?'ýK"ÛÉ/?pQç º?ï =9hÎÃ?¤2úíLQ?›øXÌï¬?¤2úíLQ?秼ÃþF?ÏÏäªö'?а†yÆt?ÏÏäªö'?çù§ jٓ?³0!u†î?Ð±¿*LÛ?³0!u†î?ìÖ	k'…?®Ãëå
X?¹O´¥	;?®Ãëå
XAGN4FGL J1727.6-3050¿Ñmk£g"Ï@@€"ÐÀ9¼'xêÍiÀ;<Zݜ'é@/§x#@ŸìÝ
Œ°?Ç~÷?×q,½ùf@	C¦GýÆ@kóā¿ï·âÅ\–?ïøÙ?Ìɝ¿ÄðÂuZõð¿åZOÈl–¿ê} >ÏH¨¿æû¼Ú'.OTHERglcTerzan 2?ê».S?Ç"Fh/?ÇÍӋF´?Ç"Fh/?è‹®@çô?Å
Ò
u×?ωÑFü`0?Å
Ò
u×?ên4å?©³ÈTh|?ÆG/ûðk?©³ÈTh|?ëHE¸ø?£åºM|L?ÂÞë±Ï?£åºM|L?؀wÓJ.?ËïóԉÀÅ?ã¿ÄtZé?ËïóԉÀÅ?Î²ÿ#êž?ÊÃgÖ~B?è|Ó@7X?ÊÃgÖ~B?ÖÁ9‡Fl?¹™"œ¹æi?äŸc<\Éý?¹™"œ¹æi?Òÿ3E–{ò?¸ì	±3ã?æ€f]4Â?¸ì	±3ãMIXED4FGL J1728.0-4606¿ØŒ5˜hA2À
çO/<À97cf×¥nÀ;-±@óL/Çn@¿Ue""?¶¯ÀøXA?Ò>¨\U†@"q VL=?ø3
ÎʨÛ?ïÿÙ¿y}¿ß$Ěúݿ჆g­Ó¿æ¥ÒWPHî¿î¸Ÿƒ¾f¿ï÷q†U7OTHERspp3FGL J1728.0-4606SNR G343.0-06.0?ÙXŠ	ÂT?Ð<S.'A?ãSºûûÖ?Ð<S.'A?Ðù"û9?ƪ¶Õ¥Ë?çõƒ7¶d?ƪ¶Õ¥Ë?ÙBňœ?µa!5J]É?ã^;±ÿ8?µa!5J]É?Ò>®‡Î|6?­D#Ч"?æ਼Áå?­D#Ч"?˜™ëÈš?™t¥ÄJGL?ï;0§µ¬?™t¥ÄJGL?ª…Úà`ÓT?·T4Ë%ã?îW¢R>ªú?·T4Ë%ã?¥©ØVä£?›]ñ²;OW?î¥bzž¶?›]ñ²;OW?!"—¬?zõý¥ä&ð?ï~öïÏÊó?zõý¥ä&ðPSR4FGL J1729.2-3641c?ï
}¾"¿ôŸ(NÓ£À8Q•p?-<À:LÁ¬Zg@·
Rê2¹@ríãÉª?¿z—˹&}?Àp£$è@SÍÅ@Ñwò)þ?ïà!sNÑ¿áˆ8õë¿ákz¢]z¿éOJ@ì¿âŒÍ}÷§—¿ë	—"ÆÔeOTHERunk1FGL J1729.1-3641cNVSS J172917-364008?ëðñ¹ãˆr?Å*4­öQ?À<9qÞ6?Å*4­öQ?í"ýý`,T?¶$¥õÊ&?³X"¶^?¶$¥õÊ&?ä%
ÅTLL?¹ä·ü»e?×µäuWgg?¹ä·ü»e?í<¢ Œù‰?™'–÷ó?¶îû*@6?™'–÷ó?äu+kȅ?Ï	ð7ì?ש)Ún÷?Ï	ð7ì?ä®,âra®?Ò
»u6Ü?Ö£¦;<¥?Ò
»u6Ü?ã·Ôïö?¿†~´»Þé?ÙؑôV ?¿†~´»Þé?ÙÃõo1?Á[6‡{Š?ãvHqç?Á[6‡{Š$MIXED4FGL J1729.9-2403¿äßÖâá@@]•ÝLwÀ9s†öÿ¦À;)½¥œà@̏›"ï·@ìB 6m?È{™=´?â}
!P² @"‰|ëãé?þéÁ¢w8Ç?ïü×÷£:,¿ÔÌÕUc¿ã¤¡Ý5¿ëÿ‰b"ʨ¿ïõê28ap¿ïù)¢ßÇOTHERunk3FGL J1729.7-24081RXS J173013.1-240234?³È‹
~‡‰?Æ*u)LÕq?í†îžP/?Æ*u)LÕq?·ù%w1/?ºª¾ÅxÂ?íÛPâàN?ºª¾ÅxÂ?Ӏƒ+^þ?³'RñàÀ?æ?¾qjP?³'RñàÀ?´íYÓ8ªI?™AZRà?íbTŘê·?™AZRà?Æ¿ÆTÈ?Ï¥ZçŠÇ?ê|jüÎ?Ï¥ZçŠÇ?…õlL¸?œŒÂGmè?ï«Ì)ÂNÍ?œŒÂGmè?²¯¿À7ò?£¡§§p¿'?íªŒ±1?£¡§§p¿'?eJÄ<b?T[…´Ý?ïêðæÔØ+?T[…´ÝPSR4FGL J1730.1-3422¿Ë£ë+²‹¿ÂGUêmFªÀ8¦Žt¢À9šÍÔ3É[@¡Ìzd@½Ofo ¢?ÍØ&ݏg¼?Õëòa±ËÀ@'؈v\?ö¨Z†¬Ø¿Ü«®¤Ã™G?ﬥDȆí¿åހ¾×@Ä¿éclK'µR¿íT¿	•ªø?"Ö9`°*OTHERunkNVSS J173013-342115?æû
pØkx?ӝ²~©"?Ò	ëO)?ӝ²~©"?Ó@›0rŽ"?Ìq°'+?æ_²gƸ·?Ìq°'+?àA$=]??¶ó÷…)H?ß}õ·…E'?¶ó÷…)H?Ð
å™âœ?²dÚêl¦å?çú3sŽ²?²dÚêl¦å?ç,N›!7?Òó
®"Rˆ?Ñç§bɽ"?Òó
®"Rˆ?¡M™Ü#P?¯¢1¬k?îë&o‰{?¯¢1¬k?̃Ÿ1^?±ÔqÞ—?èùŸ3¨y?±ÔqÞ—?sÔék³ì"?j"éu=p?ïØV-^2?j"éu=pMIXED4FGL J1731.2-3234¿îdz§'?å$Ðd1À8yÃ
0j+À:?–fß2*@`¿ÞQÚ@,€"Þ?¿^•–Ö?ÓhOŸ¥wH@»4¾?ù@w?ïÂ*|«LJ¿Ö"¦%=d¿àã7r]¿ãÕ¡Qô¿Z¿íoJpfši¿ïÿ¸aÛ½+OTHERspp2FGL J1731.6-3234cSNR G355.4+00.7?¶Ž¼jÛ¿O?Á^*,Ï@ð?í.(rmŽV?Á^*,Ï@ð?ÆhTÊ?ÀùBb'?êeêÍ`<ù?ÀùBb'?Ì`ÍÜRŒü?±ƒ¯.
½9?èç̈ë\Á?±ƒ¯.
½9?ÉhÌ88'Ó?ªšCöjy?é¥Ìññۋ?ªšCöjy?'3á'15?³¤ñŸ<?ïs–`æ0?³¤ñŸ<?'ƒË0}g?˜ú¿aDâŠ?ïoá´:…?˜ú¿aDâŠ?™Qa†'­á?†ó™ãq?ï5tóê?q?†ó™ãq?z‹ (Ê9£?hoŠ8gú_?ïÊè¿z1}?hoŠ8gú_PSR4FGL J1731.7-3445¿²Û\ª_kt¿ãØJ¯P»À9£££Þ–úÀ:ÍÛÌDÑ@!ö]¥øw @mŸ¸—Œ?ÂxžözÆ¿¦ÉÍÂÐ?é÷3]z"@û»!ԑ?¢·µ8†">?è–._äÂ¿è‰ù¥ôò¿ß''%οêNûæ•Ë¯¿†WýS8OTHERsppSNR G353.6-00.7?ïj=´Ò–L?¬äò¶Õå[?'¸I`…Ì"?¬äò¶Õå[?ï¬îMمK?–ÿÛ×?"Äl—]J?–ÿÛ×?íp,Dº´?¥réJáð?´~ŸvHà?¥réJáð?ï¹ùÙL?qdì8®å_?¸Êõ?qdì8®å_?ڰæ?¨EMwc+!?¤wòXa:ä?¨EMwc+!?î.[÷¼S?ºx¾îëæ?®?¨SÊ?ºx¾îëæ?ìJ>L8_9?§ê¨qLA?½®
ž=5?§ê¨qLA?í¼BæPùº?¥Ó¦:ÿ¿Å?²èËÀd2?¥Ó¦:ÿ¿ÅAGN4FGL J1732.8-3725?ì¯;íAŽÀCÁð`À9eV2;¼oÀ:ìÍ҆J1@"~'¶Ñ@åH©¼ýL?ÑSÇ'q^?ÏmŽä3ñŸ@ˆÚ¶š[@?¯uxýî¿í$Ò°+¬?ïõ9Ó`dÅ¿èê$@ÒA¿ä—™^á6ç¿éÿD^(Õ6¿çÃlfZ§ìOTHERunk1RXS J173250.4-372144?ïk
/XÞ?›*¼kC?'žº§¦?›*¼kC?ëý¼Ò6v½?¾"H‡á¾Õ?À	·&%?¾"H‡á¾Õ?ì_q¬·ûÒ?¦¹âªÓªl?½rš@!r?¦¹âªÓªl?íDº/'=?œC04ï|?µß/ÍP•?œC04ï|?éõY |¯ ?Ã-»36'?È*™~
C'?Ã-»36'?ßU:¥Ôv¡?ÓâˆtÇìØ?àUb­Ä°?ÓâˆtÇìØ?Ý[Ž¢€Ú?ºˆºÏ+*?áR8®¿'õ?ºˆºÏ+*?Õ<‰Ænl?¿ÄFô䡈?åa»uÈÊ?¿ÄFô䡈	MIXED4FGL J1733.7-4734¿ì )ZHÙÀ@š$À9ô§5jEÀ<Tsõ›@ ÂÄT­×@ÔF=Ñó?´Ÿ&y¿°ÒÖ|#'@Òß5…@h]‡º;?ïûw¾Q4¿àÝe4Ù&¿ë¢=aàDÏ¿¬ø[EöÚ<¿Úìé7fž›¿Ýã_ ÏmçOTHERsnrSNR G343.0-06.0?ïú´,©˜?@.Ÿ"X?E/MþsìF?@.Ÿ"X?ïÛô·;Yâ?‹Ý³Ö5?r¤?ŠÎ?‹Ý³Ö5?ï֒2òñz?y½\['qe?t¶æf{!?y½\['qe?ïð(2½Ü3?EoÝç3h?_¯šGÎz"?EoÝç3h?ïì#ƒ™?c¸É©'€?cÜ|^ʌ"?c¸É©'€?ïòȁ¨?°çš!Œ"9?!¦þ7ý?°çš!Œ"9?ïywô"x.?wèÍg$?ÑtP2=?wèÍg$?ï‹1ƒL?~N"¢eA?3¿{½?~N"¢eAAGN4FGL J1735.7-3026?ëJ
iø ?ðZ|MXxgÀ9êCÖ¦À;Ô#£s7/@Ã՟.Y@âñíÅï?ȃ§¿Í
?ïÿ¼¾ŒÃ@ÖþqŠ†×?ö39=cc¿ïø⚔k¿ï|˜6Ã
¬?ïÿ÷fÔJp¿ßhóžó ¡¿îÈ3'˜¿ïÿyýò߆OTHERglcTerzan 1?¡öñ—.O?»p–7‡?îàæ
?»p–7‡?µÎA7 Ô?°ðÃÔA‰?íF7Øð'Æ?°ðÃÔA‰?ÌÈëýжø?°d5™ìá?èÍÅ‹ÒB?°d5™ìá?":½Pºûè?sÜ`+{¹?ï¯
—øI?sÜ`+{¹?Ò6¼h·¶?×þVvs?æäý!ˤ%?×þVvs?"
G-´?ˆ2Ž!Âj?ï¯Öã¸1ñ?ˆ2Ž!Âj?Æ5O'§v–?²GÕLeB×?êr¬–"[?²GÕLeB×?6Œè\/"?6üpôµÐ?ïý'MvÖK?6üpôµÐPSR4FGL J1735.9-3342¿ï´<*'Æÿè¼Ý W
ƒÀ:I¡òYNÀ;•ð	÷y@$>ìW¬@?öúReŽÐ?Òõº+àY?¿/øìˆ?昏Bþ'Q@L¨–a«Â¿ÙÝ>‰þq?ìÕ¨]ס'¿ë¶y¿¾ë¿àt¹°V$¿ÚC©blD?¹kt~hLOTHERsppSNR G354.8-00.8?ïý"ìZÔ?=	®	»Ã´?7ÛÙçÞ?=	®	»Ã´?ïѝþ|ñ?€+8±Û?w1ԕ[Û?€+8±Û?ïˆ*xp÷[?‰š™/?õaÜâñ1?‰š™/?ïê{OñHÇ?ZåÛEôG?e"° •1
?ZåÛEôG?ïé,ðµ?s'˜û?fÓ6GÈh?s'˜û?îì5Žçå?²3‰†ôGÝ?¡<®†5š´?²3‰†ôGÝ?팋jƌ0?ª2ïè?³›¤«ƒl€?ª2ïè?Ušb?‡«èG—a?Œ^j™{ç'?‡«èG—aAGN4FGL J1736.1-2628?áÛ6:	ø@Ž)#øÁÀ9Ë~>Ê@+À;!ë¾íç@8Å]F­@"¨~8ë?Ò.!%"?ގÍbÉÎÁ@z?|ÑÔ?ø@ƹã;#¿ïýV½{öñ?ïþ¤ ³¿5¿è3«=°å'¿æÌü¿ïù÷<âß^¿ïö.$ÖyOTHERunk1RXS J173614.4-262806?éƒS¢êP?ËÂúcçc°?ÉóŠ±tV¿?ËÂúcçc°?Æë`ý`á?ľ|tg'y?êE'üÀ§È?ľ|tg'y?æ³hž`9?±fKʔõV?ҙ.Ã?è?±fKʔõV?ÓJûðë~Ø?±7õ‹nó?æZ'Š@"?±7õ‹nó?ç\Ï
f<l?Νr³¢?ÑFaå3‡'?Νr³¢?'÷D3zo¢?¨²Uº2£?ïhEÞtS?¨²Uº2£?Ò¿5ljÙµ?³édíßN×?æ eIʓ%?³édíßN×?Ž.d
yR?/	¶Â´?Fb«?/	¶Â´MIXED4FGL J1736.2-4443?ïÿtŽaÀç"~§¥ÌÀ8¶A+Cz©À;›<Õsd|@4ê³èzR@.Oü—•³?®éùOÛ¤?×{z«í¯@%	¼râv@n¦R9³«?ïóÝ£C<¿³3ãu!¿Ü<Î<Ž{®¿åp³[â~æ¿ï ‰bi׊¿ïõ8%á;OTHERglc3FGL J1736.2-4444NGC 6388?b+?œÁ¢è?e¿…Ÿ8Ua?ïíÔÀr\¥?e¿…Ÿ8Ua?¼{×ä\?¹Txh¡ž?ìp…}ãt?¹Txh¡ž?§ÏÆ"ž?œÅ†…¶Oí?¬9@?œÅ†…¶Oí?ª…Ÿîp¬(?™;jÒ@[
?îW¦ýx^?™;jÒ@[
?bD¢ˆõj?|TËÎeú>?ïí»]ŸÔ'?|TËÎeú>?—ÎÐÀÉʔ? p+"]à?ïA‰yÞ4Ì? p+"]à?†EŽüóá-?sڋHÀZ›?ï¦éÃþr?sڋHÀZ›?OÅÎ¥f?D*õcä?ïøŒŠ½^?D*õcäPSR4FGL J1736.4-4052¿ï«îÔ<5nÀÔÖ¡aä÷À:PfiÁdºÀ;¿ÎçY@@XÍq7zÁ@²£Üºî?ÈPG@0q¸?·ÀÙú]?ò4Íg&Ç?þ"š™ÉÀ¿à,ƒì‰*·¿âò2ý®A¿íå*ýÌ=?Ó©£Ò؈¿åàÝPþu¿æ!μ'gOTHERunk1RXS J173638.5-405203?ïùßêXE^?H%GYÛ2?H€VÚJ.Ö?H%GYÛ2?ïÍnãª?…¥q¸*ß?ywȑéFâ?…¥q¸*ß?ïªACä}»?"õ's"?…o¯à'G?"õ's"?ïíãa¨€V?L7щ½?bžœ7ً?L7щ½?ïçP	"ã³?k•~wï@»?h¯öT¾ôÌ?k•~wï@»?î˜Øª9>?¶7çá8‰?¦rv$€…$?¶7çá8‰?ïН*·}?•M*¦ï.?œ¥ìXñBT?•M*¦ï.?ï?³ÍU†?Ž¬ùWK>¸?˜	†X͋4?Ž¬ùWK>¸AGN4FGL J1737.5-0313¿éitäÖ@-§C"º"À:{i³"ÜÀ<7dè·äÞ@ÆUhgG@üó:õŸT?ˬñ»ÅI?âʹaµý}@žŸj"ò'@
Þ4(Q¿æ²®¨õW0?ïȳBb%9¿Ï_Qߛ±w¿éQß@lך¿ïÿY¢Ò1¿ê8PV×OTHERglcNGC 6402?ßÇ76¢ÿ?ÌY©èNæö?àudd®€?ÌY©èNæö?ØÆÎ3\×O?ËZ
1 "N?㜘æQ"X?ËZ
1 "N?ãûO¢æ°Š?³˜CTfÕ9?Ø	`º2žì?³˜CTfÕ9?â]ZƒP¤U?­0Ì¿uq'?ÛEJù^·W?­0Ì¿uq'?³8%Gæˆ0?»g(B¿BK?í˜ûW,jJ?»g(B¿BK?±ªŒ½àm5?¿ÐWWèÂ?íÊ®hCòY?¿ÐWWèÂ?·ç	-q?¦Piàê?íÚzy2?¦Piàê?¾h*w\?¦"þ±îœx?ì2ú¼|Ñ?¦"þ±îœxMIXED4FGL J1739.6-3155?ËžP|^¿Þp"ýþs
À8¤nM]À:X"@pǎŸj"@	:ß.Ï d@_å Ù(ü?×6þ™Îs@´ebZh+?ÿ
¢ÕØd?ܪ(][Œ¿åAxÀÛý¿ènrÚ/­¿ì,` ÿ"u¿ä}C!½¿ê¿ä§Œ¡c'wOTHERsppSNR G356.3-00.3?êFBÀ«?ÍÆúòÇU?ŊæôýS¹?ÍÆúòÇU?ãǕüè.¹?ÒÉFa§ÿ?ØpÔ/¢Ž?ÒÉFa§ÿ?པË~™
?¶}ÕŸs?ބÖiÍæ?¶}ÕŸs?榍?ïX?Á§nC†ž?Ò²å€!ùO?Á§nC†ž?åYŸ5ºÌð?ҙÝC3þ­?ÕLÁ"Šf ?ҙÝC3þ­?Å%	9d¥œ?Ì~N…®?궽±¦Ö™?Ì~N…®?ÞA¾!Ÿs?¸å­ð	?àú_ ï0F?¸å­ð	?­Ý%<S*?¶'MG'ƒ?î"-¬-}?¶'MG'ƒMIXED4FGL J1740.3-3058c?ì}¿¹=ù¶¿ºÒ¥ÿ®vuÀ7ès¥ê
À9¥€!ùO@š.êÏ@E×_ÍÅñ?Ǿ%ÀÕ?ДΣç{O@çžóu®?ó»›~ñ"?ì.¿eÛüë¿ÓƼýÌÉó¿æT%B|¿èm`öºÜà¿éÆ&Tþ_¿áº­EH­OTHERsnr3FGL J1741.1-3053MSH 17-39?àWM=dSV?Ô¶)ŠñhÁ?ßQe…7YU?Ô¶)ŠñhÁ?Ï·ËÄö$ñ?Çôêv£p?è
ÂvÄ?Çôêv£p?Ú îøpÀ?·wAö‡–?âþ/ˆƒÇ ?·wAö‡–?ÂùpÓÁws?¨j=@;?ëA£Ë¢#?¨j=@;?áÐZº¥r?Ö8â°Êõ?ÝÒ_JŠµ?Ö8â°Êõ?žæùpZ5J?«rd¼ç(M?ïÈ4¦i¥?«rd¼ç(M?Å°'åøý?°ÌR¢þáâ?ê"öúA?°ÌR¢þáâ?eÑIPÜ\|?]%5¾ÂÐ?ïê.¶»';?]%5¾ÂÐ0MIXED4FGL J1741.1-5341?Üü«\d¯ØÀ(¨"1¡À:1ôú€5À;¼K±¯:@n¢ÔUØ$@t£%3–0?ʏ`Fþ?Ä(©båR?ø'›k*ñE@MGva0G¿ÑßrV^±f¿éQK·Žw'¿ä€–ÉÁ0¿ç||Šiü¿í^æ¤h¿ïþÞ&'dOTHERglcNGC 6397?ïÆhܯ»;?˜$"°?^¡?|ˑ#¢T?˜$"°?^¡?ï½À§nŒ?‹~8Œ…×<?€Ö=ä
?‹~8Œ…×<?ï:Éxô!?Ž¤I¬ä}'?˜¼†ËºÚ?Ž¤I¬ä}'?ï·³`­-?eLôåA¦$?''Þl
®?eLôåA¦$?ï=ß®ö¬?–
´SèR?˜D$ùÀ"?–
´SèR?îɕNŽr?°¿ÿ¡Ë?£f®§|á?°¿ÿ¡Ë?ë«¡:Ý?­vlñW?ÁQ{Ï‹ä?­vlñW?ìëHxó9|?¤/—	€ä?¸¥¼8Ô'¢?¤/—	€äAGN4FGL J1741.4-3046c?ïrÎ0±+¿Éú³åË zÀ9MÛ:MÙ¨À:ØZ@ä@[¸b‡Š@Q¬šþ?Ò±–¡]³?èzÎg×®@à‰ï•O?ÿ³'ú;ñ?͇…oëö¿àZ[–(Ì?×4AðeX¿å"†bZ=8¿ê'Ì®š¿ïÿôým~‰OTHERunk3FGL J1741.1-3053NVSS J174122-304712?Õ`%Êiñ
?Ï	#6³?åOíË{?Ï	#6³?Ô;ñó£?Ç¢48Òë†?åòvb/?Ç¢48Òë†?àFu‹%A?³2r!%V¶?ßséµÕ~?³2r!%V¶?Òð}hê?±‡p`Ò?æ‡ûöAK‹?±‡p`Ò?ÈRÞãêd?˖ЂË?éþ+HGg?˖ЂË?¢>¸ž'Ùõ?¯±Ù§1Ïß?îÜuØÊ1?¯±Ù§1Ïß?ÃIºSxx?±fLh?ë-'k!áý?±fLh?š¶zné¿7?n]´CÈ?ï*L,±íV?n]´CÈ0MIXED4FGL J1744.5-2612¿âñH"K@?ú«‰†&À9
	A}À:Óeµf~º@©Wn¦Ñ»@'û'½?Á}Žá"¿Ã?¸?YV†J?ù•œdO4ñ@2¯Õ›'Ž¿¶̶Q‹8?ïãšn«¯¿æ÷?ö:.¿åµŽÚù¶¿äÁN·8¿ÜžWn{ޞOTHERunk1RXS J174419.9-261230?ïÈý†]¢?­¤eÿE?{=ÞrÝ?­¤eÿE?îž@O{hV?°Óaó?¦ûm"Ÿ?°Óaó?í܂›|?¤öѪ˜tŸ?±ï$ߊ?¤öѪ˜tŸ?îãN3ó*7?†\µXT|?¡ËÃa‰?†\µXT|?ŊÊZ?ªœúËXp"?¥æ£¨/A^?ªœúËXp"?äÝ~T|Ñ?ь`-Ä?ÖEÑW]?ь`-Ä?ëyb×]ý?³ƒðª(†R?Ât¢‹¨?³ƒðª(†R?謁Mûéù?¶'ªq¡+?ÍMúÈX?¶'ªq¡+AGN4FGL J1745.6-2859¿Îqˆ\Ê7¿£ï›ƒÔ‹]À5–åápÈÀÀ8ïlÒÐ@ "_§ÛPÉ@…+%G¸%?˜…ö¤Œ'É?ÅÄ¿b+]@/
'Ä"Bh?î•‹Â|£¿ÀÎÊ}è
E¿Ú@ "®¿à&cvÇÝz¿åßEuU¿é<ëج¿äç›O|?OTHERspp3FGL J1745.6-2859cGalactic Centre?ÖlCiØû?Úcþ'A¶"?äÉÞvK'?Úcþ'A¶"?¬Åæ›ÙO?¦¶}äƒä?î>áÍ<+?¦¶}äƒä?Òp‰Lg?´LF$Ÿ:?æÀ{Ç»YÍ?´LF$Ÿ:>î9¥`ªR©>ìïlˆaëñ?ïÿáƝÍu>ìïlˆaëñ?ÛS2ÌëÂ?ځ|¨ƒS?âVf™ðŠ?ځ|¨ƒS?€¨‹aãîÔ?"~Ž\kê?ï½]ÒO}?"~Ž\kê?Ç=%	NÞ?¸$ZÇÖÇ?ê0¸6½¬H?¸$ZÇÖÇ>=ªg%ؼ•>HsYmI?ïÿÿü=íe>HsYmIPSR4FGL J1745.7-2506¿ï¤»=O¹?ÿn$…ñF)À:,]VlÀ;À9'ÈÅ@'9òj@yÁ­?ÔöíM"‡?'xë¤@ä5À¬-?úϽ<¶ê¿ïþ~üà;?ïý±Ü†~4¿ÆÐîÚ雿ê¸1Ûã@¿ëð`"=µ¿ðOTHERunk1RXS J174535.1-250440?ÉÿÒ(z#?ÊVh#wJÝ?é€uÿáw?ÊVh#wJÝ?¿òÕ¨œ?À«îÛÀZ¤?ì¥Jì|.?À«îÛÀZ¤?ào3ÜrԀ?³k¼ˆ(z?ß!˜GVÿ?³k¼ˆ(z?±Ü×à¨×?š
¨ò)?íÄeÝ&¯?š
¨ò)?«cü–Îj?ÄÀ Ÿ\?îIÀ6wœ€?ÄÀ Ÿ\?†yî=ÕÜ?›œ¡æäù?ï¦FâY?›œ¡æäù?¿¢Ë¾Ò/°?ª…"5&?즈%º
?ª…"5&?oM2úƒ÷?_Ö_ÇIs?ïà²Í»ì?_Ö_ÇIsMIXED4FGL J1746.2-3342c¿ál×m©jŒÀºAå}»À9¬.þñGÀ;ÑÙ|¸@ôÔ$"ï"@Çz³$…?Ð졾×Ñ?¬Mîd;Í?ç+8ÞøÅ@JÏz?ï~E뜛­?˜¢"ŠwE¿ê)æž/*¿äDïž3h¿Ý
Š2‰~¿ßÃ	Õk׿OTHERsppSNR G355.9-02.5?ïïDzú)?k>ÙMC?`8MöÄG6?k>ÙMC?ïڀ/¡iƒ?çyւ?r¿èAÙ"u?çyւ?ïD ßQ<f?"‡—rÿ¥2?—{äù;A?"‡—rÿ¥2?ïï°æÖýí?Gã/I;?`Oóh+[?Gã/I;?ïÑôha<?'õ¹v—?wËƐfK?'õ¹v—?ïBøÅp"?°Iò,üº?ž7 î1'i?°Iò,üº?î]
a½_G? l÷ÂGLk?ª/)ßވ? l÷ÂGLk?ïv¶lÛlð?":Pô½>S?')2]³*?":Pô½>S!AGN4FGL J1746.4-2852?ŠùÌ=¿½¯+ÀçÖÀ7b·«cÀ9¨ä:§›»@ €$±0d@­ÿYçÒã?¹²Dxªâ?æGa=‡Ÿò@'¡"¬S±?ÿò©ëJ¿ïÿÖ_Æ	?ïÿu–…#¿É"£{Ѹ¿á͚ݼ^@¿ì–à­F¿ëÿfèle"OTHERpwn3FGL J1746.3-2851cPWN G0.13-0.11?rÙÐ&¯¨`?®ßäï'ÑR?ïÚL_² ¯?®ßäï'ÑR?¢Ïϯ¬á?­sŠ9Ÿ÷?îÖ# '?­sŠ9Ÿ÷?±"u™§^é?¢Eç‡6‹D?íÍqLôOs?¢Eç‡6‹D?â×üÓd?iæQÍä+?ïÿéÖÊ?iæQÍä+?­N{ýÁ%>?Èo~õËÁ?î+@#í¬?Èo~õËÁ?nD4p˞<?"¨ªÍ0?ïá»ËŒt²?"¨ªÍ0?¯+е±õ}?£47Ñ8Ól?î
Bô¤à¨?£47Ñ8Ól>Ž€AoŠ >w
g#k?ïÿÿ‡½¬§>w
g#kPSR4FGL J1748.0-2446¿èg£Ho?û&òIÀ7C¼¾aÐÀ:ˆ?›÷Aë@H@
²@ú¦Kaþ?¢ô2ÂJò?Ö'½3Q¼@0¹:>À/0?ú¢3'ÒÑ?î°Ý$•¿Ñp*
ag¿Ýù˜kñk¿ä¸–IƒÑ¿í_›¦º¿ëVxHOTHERglc3FGL J1748.0-2447Terzan 5?/0ŽÎâ܉?4ájÀ±$?ïþ÷E'|?4ájÀ±$?™A:á<?¤J#ä±|?ï7õöDrÿ?¤J#ä±|?Žð7֞]?lM÷}Ò?ï"? Á†?lM÷}Ò>þ5?²•‹ÿ>üB¥Q/¹f?ïÿÕI0~>üB¥Q/¹f?TB÷â½?cè]Šo£?ïõބbÙG?cè]Šo£?c]ìC±lá?v.–d/¨X?ï좪p›?v.–d/¨X?Œjy"˜2N?‰A–{Á'=?ïŽV'"W?‰A–{Á'=>d_¤Ä1&}>uÍå¦	h¸?ïÿÿë™QÜ>uÍå¦	h¸PSR4FGL J1748.9-2021?½jy4@Ç@X䓒ïÀ8íÿS1Ö<À:ä	EùßU@§ïŠçÐ@¤ê/´?¸(^ÿûßp?Ò—=í§@=Ÿ¿MˆI@Åì•j
?΀%)ZAj¿ªnSà&ò¿àê:†ä‹¿çt7ª'8¢¿ê_gJ¹¿ê¼2€…Ì]OTHERglc3FGL J1748.9-2021NGC 6440?Î|òþÔu§?Ȥ$†‹ä"?è`Ã@Jâ–?Ȥ$†‹ä"?Á0;ǁ^d?¾¹^E…›5?ë³ñ¨g?¾¹^E…›5?àAëâU?µma«ú@å?ß}(;Tâ?µma«ú@å?Ճì;ۀø?¬I`Sú>z?å>	â?"?¬I`Sú>z?v?­
Jî?‰"KshNë?ïӁþƒR?‰"KshNë?ƒހ#\ï?'C§ôW)?ï³ä…ÈxÍ?'C§ôW)?¥7ðo.Û?=,8öŸ7?ù(/?=,8öŸ7?'ù¯®ÙDz?z½V±îGA?ïp2'‰1Â?z½V±îGAMIXED4FGL J1749.5-2747?ÁôÀ9t'¿Â1²ªŒ°þÀ9yòìòBÀ;gÝkí@Õ±šl(@mZ˜?тl¡"ãø?ïÚø4H‡@~x?'æ?ô‡×¾˜?ï5ø_w´Â¿Ó'óÂÚۃ?åDª¿[Ë¿âÕub'¬¿ì/bCA¿ïþŒ}QdwOTHERsnrSNR G001.4-00.1?ÂÙêlšÝç?Çç0-ø¿M?ëI…dÙH†?Çç0-ø¿M?±F·¨5¸?·ÒÍAç«ö?í×)Ý:Ù?·ÒÍAç«ö?ѳ3"ž?¯†0þrÉ?çw¦fun±?¯†0þrÉ?v=ÑÐJcY?dú
É5×;?ïӄ\¤#i?dú
É5×;?ÃÑ6Ħ?Ð+Úe«o?ë¹òŽÖ?Ð+Úe«o?'íoċ?"ñ iR^?ïÀÚ$ƀO?"ñ iR^?¾W…@#å?¨N>o›Q?ì5Wûƒ]?¨N>o›Q?8 ¦®Û|?5V/ÛÙ1?ïüëëmn:?5V/ÛÙ1PSR4FGL J1750.3-3702¿¾!ÈoÎw¥Àäõ8À8êõÚPÀ;RՔ«@&¦ßh±@'~D©}<?³éçdӔ<?ÑçäÀ´e£@AkÛm@ÚԏŽÓÃ?ïÿ6A­?ÍÝ%OšÈ¿ã
œ5ULc¿ç4"䤿ë68Öá"Å¿åȊ³LÉOTHERglc3FGL J1750.2-3704NGC 6441?ƾ¬<xE?ʽ%ê?ù?êyPTðáï?ʽ%ê?ù?ÎÁíUƒj-?ŜºYÐ?èO"ªŸ%u?ŜºYÐ?Ú.Ø,sÈÇ?¶9µênY‹?âè"éƝ?¶9µênY‹?Ø$æ¹ÝÜÀ?³,9›'a?ã팣 ?³,9›'a?šLaùv?¡èÛ¥Ï?ï+…œây\?¡èÛ¥Ï?§WÍþk¤?´å½,jè?;–&?´å½,jè?š
¸3êf†?'âU£Š.#?ï/'>Rî\?'âU£Š.#?•ÿÕ|‰?'ʪ댽?ïPT`Kè?'ʪ댽PSR4FGL J1750.4-3023?Ú-Ѩøî¿ú'Ã^À9÷q'ÒüÀ;hšQO}í@º†è¼í@Q~B%>~?ÒËUhè æ?寡]³9~@lğá§?þxqƒzô=?¬Ç‰£'Q?á¶úc
¿¿òØ`eÇ¿è¦Æ¨Æ]G¿ë7V]Ú¦ª¿ïïwAU	óOTHERunk1RXS J175019.0-302654?îQÖ¿óS?±.~ GrU?®Šâ"$ãÏ?±.~ GrU?äút<Ðú?Ǟ›–Éہ?Ö‡þ^?Ǟ›–Éہ?éÌRŽ' ?ª¥º©Ó†L?Èη™Åõ~?ª¥º©Ó†L?åQøÈÔÈ?¬bXíÕ?Õ\nWÌp?¬bXíÕ?æ€i3G;?Ì^vzR#?Òÿ-û™q‰?Ì^vzR#?ÂòüA?ÄÓ{
xŸµ?ëC?ÄÓ{
xŸµ?Ù|´Z~ë\?¸hö—ª	?ãA¥ÒÀŠR?¸hö—ª	?Ãò
7Öõ?¦í_
ôÈ?ë}r
xC?¦í_
ôÈMIXED4FGL J1750.8-3106?ê¬>	Ù{:ÀÊ÷?gÀ:h²qôÀ;®†Ô@o|—@V[~«×Š?ÓTo—4?ìϵIùHV@©ôafLe@Ù –¦¿æE"~°	H?ï‹ÈUnÇ^¿Xøš$W"¿åÇ-»úír¿îÁÛ!yLr¿Ú–Ý&·#îOTHERunk1RXS J175042.7-310312?ã²VË­È?ÍYi¤oœ¬?؛Rh¤üq?ÍYi¤oœ¬?à"à—ÿT?Ì6%²R^X?ߺx¾ÐW?Ì6%²R^X?ã-‰ÑƒŠ?²»r‹9ŽÕ?Ù¤ì\ùÄì?²»r‹9ŽÕ?ޓ;y±Ov?³	hµ¾@Ø?à¶bC'XE?³	hµ¾@Ø?ÒPµ‰(! ?Íò.í9?æ×¥;kïp?Íò.í9?µŠÄwÓF?¾ù…
V»à?íN§q.ҍ?¾ù…
V»à?Ď
¯±^?°Xè÷SGË?êÜ|}T¨?°Xè÷SGË?±0C7vߑ?›_ܹÓ¸?íÙ÷™:_^?›_ܹÓ¸MIXED4FGL J1753.2-2848?â9Ž<_¿õ¶2ŒDFÀ:^ıuXÀ;RU.‹.@'Ê'š¤‡@8Ã`<€º?×íK<¿N	?賁6ÌDè@
*=DŸ@‹¤íµ¥"?ì€BŠ3ö¿ç)BïhÙ¿Ó•j \×F¿ã«LŸjéÙ¿ïÿ»×²¿ÜŽÂÛ²BÞOTHERunk1RXS J175328.7-285014?á 9{»|?Ñ$ôÄ/?ݿ͍‰?Ñ$ôÄ/?ÖýŸ¬Çãs?ÌãÃß=gÀ?ä0)œG?ÌãÃß=gÀ?åƒ>óÓc?²º¶?ò¨6?Ôù'YÏ:?²º¶?ò¨6?ÝHm†Z†?²ÊpYUó?á[É<Ò÷½?²ÊpYUó?ÕØâTstÂ?҇¶5dC?åŽÕÆEŸ?҇¶5dC?¢·¡ô/\ý?µOÜ"v?îԅࡍP?µOÜ"v?Ñ"ZX7[?·±·_·§?çnÒÓ÷äS?·±·_·§?­†ç~=˜s?™~èúfS?î''ˆh	?™~èúfSMIXED4FGL J1754.4-2649¿îCL®.|¿ãåjR"À8ôç¸5fÀ:R¦'¦`Q@T\>D^T@(obŽj'?ÊÉÓH<ç?À˜|¹)?ü}[
Ѻ?ö­…¼?ïÿ%¿Ø·¿æo—@G¿æQî¿æµV¿ç¦üX«'À¿ä'/ÿÌÿM¿æQµ4)Ó8OTHERunk1RXS J175501.7-264954?äRE Ú;Ü?Ô¡¬rº1À?×[t¾KˆG?Ô¡¬rº1À?á/¢ªïÐ?ΐxl½u?Ý º«ô _?ΐxl½u?ã:Tâ?¸­Öƒk3?ًÑËËV;?¸­Öƒk3?ç0c§0ë?°ÂŸ¯Á?џ8±ïž*?°ÂŸ¯Á?á£e¸õ1?Òv
Y†jN?ܹ4Žñž?Òv
Y†jN?²˜
kí?À­ÿ["$?í¬üã5£?À­ÿ["$?áÉ«¹Æy?½^TDáí'?Ül¨Œsß?½^TDáí'?¾GJ›žp]?«r¨Žàö(?ì7¬Œ1ô?«r¨Žàö(MIXED4FGL J1755.4-2552¿êkHJëX¿Ól†á­¯À8>¡%À:"Où<—`@ ,&dä@ÙYæ%cg?Ç2>@­o9?¼Êm!¤W?þKZ;µ¸´@Û´¡ö?ïø׊•ñ¿ÚN`ÐTí¿è#¿dTh¿åÞ$ÿ¿éó`µL~¿Þ¤pMOTHERsnrSNR G003.7-00.2?坢ç'T?Ôò®2®?Ôĺä0ÛY?Ôò®2®?íš8£4¢õ?¹ÐzÊT*,?³.:ç6ÏX?¹ÐzÊT*,?âW£…D'?º¶;_g?ÛQܸõvÜ?º¶;_g?î'Éó~'?"˜åíï­?®ƒ`ÈÛ?"˜åíï­?ÜË3áj#ñ?Ñ!G.NS?ášfJî?Ñ!G.NS?âr9[žêÅ?ÓÐ]ô?ۍHÂ*v?ÓÐ]ô?ãþa6s&
?¼W¹S·üË?Ø="³ì?¼W¹S·üË?âiQbü­?¿ÑÆJ–k?Û-]:¥Ð?¿ÑÆJ–kMIXED4FGL J1756.1-2516¿×FHj8>F¿À;÷ÒßáÀ8U®mf4èÀ:!vjNR@ûHŠˆY«@À	‹û?Ã}˜F³B¸?Û[Ÿ"š‰¯@²¹šû@è*~XËs?ïÿy'3J°¿Õ:–9üÑ¿áôÌÆпëêry\ã¿êDå!ØAö¿ïÿ) 4ÓÇOTHERunkNVSS J175606-251909?ÃA'Ì+ù>?϶%Éò?ë/›Œõ°?϶%Éò?²Çb`»?·2EAe–?í¾Fø7	?·2EAe–?ϳ§P«-?²¾D'¥Í?è+Õ4¿?²¾D'¥Í?°¿«È‡è?•õˆè"fþ?íè
†ÒÓ³?•õˆè"fþ?°tÏÁ»û?Ê5Šè0?íÿÑf1Ð?Ê5Šè0?xê<ÂNª?‰wzÍàúÕ?ïÏÌ+Å´2?‰wzÍàúÕ?§(ÕÔ`Ô|?ž1â4ã?îr¢ðìx?ž1â4ã?Tq'Y$ã?F¸s"dƒ2?ïõÇl]Ö?F¸s"dƒ2PSR4FGL J1757.7-2337?îJè$?×ó*š}£À8‹
É^çÀ:¡žJÙB@ å[ºà
@ä=F²kø?ÊQù\wÐ?Å*©÷µ®£@Yí{ì
?òe@çPܑ?Ú[©ôÓ?Û&º>ƒ¿è|X@2õ÷¿á×L¸?w¿í¿5դ⣿ÀS±OTHERsppSNR G006.1+00.5?×ZËò?ÔêË-˜ó	?äRñòÿš?ÔêË-˜ó	?ÃïeC–?Ãý*ö×?ö?ë=æ¯:Ú?Ãý*ö×?ö?Úóß(w ÿ?¶ô'#»¥?â†kÄ/?¶ô'#»¥?Å Cïeur?¬Èb"Ë}?ê·ï&¢£?¬Èb"Ë}?¾µ+¹tÞØ?ħÆq?ì)ZˆÑd%?ħÆq?‹#Ê¥ú&×?¡!˜'Ü?ï"pÕLš…?¡!˜'Ü?ÔÞ°p[îÏ?¶·\8,?吧ÇÒ˜?¶·\8,?yôšNâE?pE'
œ¿&?ïÌzڀƒ?pE'
œ¿&PSR4FGL J1758.6-2404?ê<°E¾·¿£.y5}À89Vº øžÀ9þœCc@ äÄ£³xé@×î['ÍÍ?Àa×5†t¤?³sæÐ_~?þ>ɄBð@@ãJ膑ª¿éJ]ò#ž?î"Ó–ëip¿ê¦]¨R¿ÜÑÓñM5¿áçj¨† ¿í×ïunA&OTHERunk3FGL J1758.8-24021RXS J175835.5-240203?ålԙ0#?Ô¢? zc?Õ'ÐV͟¹?Ô¢? zc?ì£7÷ä?ÀE_æD˜
?ºæCxG0ã?ÀE_æD˜
?á³Ü @¬?¸B6ë«]‡?ܙæG¿~¨?¸B6ë«]‡?î%ç­ù¢ï?˜Œ:8õÆ?­¡…Ò?˜Œ:8õÆ?ÜúÈÌ7&?Óø¯3‰Å;?á'ü™äm?Óø¯3‰Å;?ájñrjøê?Óebpô›?Ý**-?Óebpô›?äׇh""ö?¿ñ«ûNÆ?ÖPñ.ÖØ?¿ñ«ûNÆ?ã/U–ñ"Î?ñ¸TÝ¢?Ù¡TÒöc?ñ¸TÝ¢MIXED4FGL J1759.1-2347c?î\ŸþÀ?OÃ%ãÀ8£hQ"1ƒÀ9Ò`8Nûç@ ½}mi
@"ã^߉h?Ô~/%1'Ê?Éèâ'q	@	Ãa@O?þþ¡ì#6¿îˆ¾ªö
?×ÒíbÄp]?ëéšbí5¿æ"¸žÂx`¿è³†_€>¿è-@ªêúµOTHERunk3FGL J1758.8-23461RXS J175851.9-234511?Ö÷&Æ
?Ô('ñó‰
?ä÷"lœò{?Ô('ñó‰
?Ó¢,?¢œ?ÎÆöÛ>*?æ.éøà.²?ÎÆöÛ>*?Õ
Á¼î‹?¸%ÝèC™ß?åy!óº?¸%ÝèC™ß?ØQy*Ÿw?ºÍ›qé"ò?ã×Cj°Dx?ºÍ›qé"ò?Ä£^<SöÖ?Ðñù,&O?ê×(pëK?Ðñù,&O?¨['•!?¹Ê_I¼ŒŽ?îzFævõˆ?¹Ê_I¼ŒŽ?Çêô6s/?´•Ç.ü?ê_'òc4?´•Ç.ü?£~ÏCJ?ŸÓ`öÌ
ì?îÈÐ}[?ŸÓ`öÌ
ì0PSR4FGL J1759.5-2312?ïD¡x=Ý?ˀæYæ¦=À8©¢ò(§À9ÐaŒâÑò@/°NÜ@ÒÇû¬´)?Ò`ÍX
?Ïϧ¹õ@	àÛ'£H?ýI"='Ûà?êo€Á[€¿èìßý+9j¿àõ\"•¬$¿ç÷ÆÀÄ*è¿æOæ'æ¿ïþ'!€-bOTHERunkNVSS J175948-230944?ÚÊà_7^?ÒèÖóí"-?⚏Ðd~Q?ÒèÖóí"-?ËáŒaø˜ƒ?ÇiÚÅ7?éœçÙß?ÇiÚÅ7?Ýmä€Xç?¸øßJ3òú?áI
¿ÓŒ|?¸øßJ3òú?Üøb
Õð?¹jüŠÏ8?áƒüNù?¹jüŠÏ8?à—ÛRelZ?Ów¸fÆ?ÞÐI[5'L?Ów¸fÆ?Ž]ß«¸]?£EÛ ¾ì?ˆ®?£EÛ ¾ì?Ù\$e‡f?»†»Æj2#?ãtQíÍ<M?»†»Æj2#?˜ì¤ÔAS?>æӅº?ï?0š°"¦?>æӅºMIXED4FGL J1759.7-2141?F¤Ð
f0?á)À8Ïa€M˜9À:ªh_dêe@Àîó[Í@¯…^y2?¼Ž½Gž¥?Ñ!šÄçÑ
@ÛHƒ&Ž@9Çóʲ?ïþ–Ž0Z¿çôÛߏG0¿Ùzßð&¿å2	g‡Î–¿êC@؍J¿íû,áàZHOTHERunk3FGL J1759.6-2141NVSS J175946-214231?Ýa†ï.1Ó?Ïþݠڀ•?áO<ˆhç?Ïþݠڀ•?Úƒ¥fi?Ëð+kéˆ?âõ¾-L¿K?Ëð+kéˆ?å|þ<u@
?µ°´hR?Õ‡æ?µ°´hR?äô±šc»^?­î‰Ð—ÀM?ÖœË8‰E?­î‰Ð—ÀM?¶^Ë'sEú?¿Òc‡d»?í4&›U±?¿Òc‡d»?¥©-µj¼?¶/r6èÅ2?î¥m$›•È?¶/r6èÅ2?ÍÂò6y?¶FNºjx?è¹Cry"?¶FNºjx?½¡öÓd@?¤šàRæ'?ìKÁ%"|8?¤šàRæ'MIXED4FGL J1800.7-2355?îõƒb—ò¿×É] í`kÀ8<Rô™špÀ9Øïÿ×¼@!º˜ó¬_š@(@Že‰?Ä6¨2¹°?²ðãB1h?üJë!L?úúŸ³ºC?îT)'°I	¿ã.ôàM/?ë^ÊÆbO€¿çSÿ[•R¿ÞI½ƒƒ­Ÿ¿é['£HoOTHERunk1FGL J1800.5-2359cNVSS J180041-235622?ٖ¹ŒËwZ?Ó©«Å–!À?ã4£9šDS?Ó©«Å–!À?äSz–I-?Ñ«R›¥¯Ê?×Y
Óm¥Ë?Ñ«R›¥¯Ê?ÜõžiJ?ºW²ïVª?á…p°þK[?ºW²ïVª?á'PÍLúZ?¾áÑIfÙÜ?ÜÛ^efM?¾áÑIfÙÜ?ÔÚþ藝Z?Õ|û.Æ"J?咀‹´1S?Õ|û.Æ"J?й×±K?ѱ8¾|?ç£x÷§[?ѱ8¾|?ܟ—îQ_w?ÉaÜÚÈN?á°4×PE?ÉaÜÚÈN?Ä|OÀÌRB?»Í¢lž[B?êàìÌëo?»Í¢lž[BMIXED4FGL J1801.3-2326e?ïjøŽ¿Ð:ÛGÀ6,l™†NcÀ8³Ïqºû@ »\æzH@B¥–ýÞ?¬¸oâTã ?ÀÁà [R@!,ÁÊ:KU@ºyŽq¿Ò1܆~3ã?ïsR4¿å•"õÎN¿ãÁè"Ïf¿é9Ò9¿âAî¢_ßOTHERSNR3FGL J1801.3-2326eW 28?""A•Ãîy?°¢¶¬Á?ïfíó
(]?°¢¶¬Á?£=} õù?¬é¬>}b?îÌ(."µQ?¬é¬>}b?Ù@D۞™*?´¼xúÒ>ˆ?ã_ݒ0³k?´¼xúÒ>ˆ?vÎt‰î?sòføÒ 3?ïº$Åöވ?sòføÒ 3?£€7ÅT•?Â}žÂ´8?îÇüƒs½g?Â}žÂ´8?mýœåe{?€éT0ȏ?ïâc²ó?€éT0ȏ?Û~Od±?¶ÝjÎCß?â@ò¿XM¨?¶ÝjÎCß?‡¦Î+Ë?¨ÌEay'?ïÿ[Ç?Þ×?¨ÌEay'PSR4FGL J1804.7-2144e¿à‹¹Ôøj_¿¸G7÷é=À7d/TbÀ9J®¯«SÖ@#*0oç@UhƓ?«R€o?î?'IR{Å?²?ïÝDêÜ0@Ë<quc.?ï÷Տ-Ú¿ÞY•‹–¢¿ç…=jĚ¿Ø9›aðµà¿áCœRæW¿Ðø3£¡ÂOTHERspp3FGL J1805.6-2136eHESS J1804-216?Ò9€''@Y?Ñÿ¾é¬£Ú?æã?·>ßÓ?Ñÿ¾é¬£Ú?ì3¨A/Ó¶?Çzlò`t?¾b½öbQ?Çzlò`t?ã0=²¹.?´'¥CñÇX?ٟ"䚍¤?´'¥CñÇX?ê•Fésvš?¶¤"LNì?ŪäZ2%—?¶¤"LNì?á~'E<?Ò:<Ñ0xˆ?ÝûÓuˆ?Ò:<Ñ0xˆ?å0ŽÙÁ4?ÓØyæmT9?՞âM}˜?ÓØyæmT9?çr†#qP?¹el#©MM?Ñó¹ÿ`?¹el#©MM?Ý/]U›'î?ÆTÀ6;{V?áhQU26‰?ÆTÀ6;{VMIXED4FGL J1805.6-2136e¿åλê§SA¿Êó› ­JÀ7cÿ¥g-6À9A¹d:<<@ Ðyšu·'@žš|îh(?·6=>Nð(?¼¾-]íWB@*{[Àðö@åŠÞÁ?ïûþQ)=¿ï÷" fQï?ï¹ý‡»¢¿äˆk%^¿æ.oŸJ2©¿â󵤒 OTHERSNR3FGL J1805.6-2136eW 30?ÈÈ&8½¥?Ï>üț˜?éÍöqЖ ?Ï>üț˜?Þʅgæ÷¤?ÒðÑOy¡?àš½L".?ÒðÑOy¡?Þ÷¬±›»T?¶t"Þ&?à")§2"V?¶t"Þ&?×Ðnïï3!?½¨öKÿ»j?äȈfp?½¨öKÿ»j?ÔǓ–º?Ò×iÅâ?åûœ64¢ý?Ò×iÅâ?ÁõtO¡í•?ÊȝóÆ`Í?낢ì"›?ÊȝóÆ`Í?âKÇçé;v?¿1Øwc…?Ûhp0-‰?¿1Øwc…?³yL—|@À?°iwªñU?íÖlç<˜?°iwªñUMIXED4FGL J1805.8-0803¿±*7*"@UÔ¥ß":À9ůJÛÆeÀ;Šꘐ@&¦7aÁ@Åêû‹üù?È}ë=PBŽ?¨}¡%ãr?ätÌ?ß ?ý­:`N?ïû¶Å#‹ ¿éh°B¨q#¿ígB'¿ÒùsÍÅ¿á	²Û‰ÿ¿ïÿ‰kVOTHERunk1RXS J180603.1-080612?"À»ê?"%µ:AÁØ?Š]Þł1œ?"%µ:AÁØ?îIŠž»(?±õš%@è?§gYƒé?±õš%@è?íÙ.
è?¡	ÈÜ¡WÞ?±6ªŸ©¾?¡	ÈÜ¡WÞ?ïf½8Q¢?z&íý¹q®?"(Xõ˯Ò?z&íý¹q®?ë4héè*e?Àû áæ©1?Ã.\X_Vl?Àû áæ©1?æ´Thb?Ï×ØJ ?җW/;×Ç?Ï×ØJ ?ëý	|Å<N?­w±Ü>Vh?ÀÚëÆ?­w±Ü>Vh?ér%_Ç!"?µÇ[›µ'C?Ê7j€ã{v?µÇ[›µ'CAGN4FGL J1806.9-2455c?íŸë¤mÀ¸Ðº%*À:o1çÙÀ;|`¾†¸ì@ÜHjÒÝ@"Á=L'©?ÔjßÇÑ:?êê!ƒ"@?úÁҝÇ@³+XžQº?ؔø T‡¿à39žeË¿É) 7mŠ¿éGF{"¿ïá=¼#1¿ïþ¼3!•|OTHERunk3FGL J1806.7-24511RXS J180700.7-245619?æ1ÿ®˜Ñ•?ÏkåmúѺ?Ӝ¢Î\Ö?ÏkåmúѺ?àRl
?Íý	œr"C?ßá[Ã'æ?Íý	œr"C?äÕø©×¼?³PdÉ†?ÖT­öP‡?³PdÉ†?㬣•Åq?±©½Â."?ئ¹ÎÔu?±©½Â."?×"Ù3bƒ?Ð,´•Ãë?än"fN¾?Ð,´•Ãë?²L":0²¸?¾u`âv?í¶m˜ðãi?¾u`âv?Øʍá:Ô?¶,ÔÛã5Ý?ãšò9b–?¶,ÔÛã5Ý?À¯/'»5?§Ðp pH?ëÔ4Q3?§Ðp pH(MIXED4FGL J1807.8-4340¿ê˜EƒdEqÀ&G2œ4~À:4I½¹3"À<àd)u@§ÏBrì@ùœÝñ¸?Ãi¦!gXÕ?Ô'r 0Œ@
NHboa?ú:š³JÕ?ïù?†þŒb¿á8ýw"¿ÛxŒÙ—¶k¿ä½þ}ÉÚT¿î–q[Œî?"E©'oÜ\OTHERglc3FGL J1807.5-4343NGC 6541?ìËR×=i?¸¥Ygê?¹¥iF·G?¸¥Ygê?ì#Wq›?À¸{SÑ>?¿žçÕDs*?À¸{SÑ>?ë4Ð'?¨]×Ü×N3?Óë,¼Õ?¨]×Ü×N3?í"&Ÿ•ËÉ?"c~ï8 r?³fËÇ>?"c~ï8 r?ä¬
kç?ȳÕǔ¡?Ö§åù)Þ1?ȳÕǔ¡?Õ‰¯…'û?ÎedF.@8?åx»(=>'?ÎedF.@8?á5䀝Ÿ8?ºŸ£ô¼U?ݔ6þÄÁ'?ºŸ£ô¼U?àòô¡Ÿo?·Lhz/?Þà¼Á"?·Lhz/MIXED4FGL J1808.8-1949c¿ÝPxυË?]ÐСõ\À8ˆF"
qÀ9¶¡Ú°»@ –îE1b@àM/^?ö£©Ø«þ ?Ôôqâ'Ò@Ãñ[øN[?ø±÷¤;Þþ?ç:¶#£s?îêÖ£d!¿èÛLAw»¿êKåM¸¿çqµºa>¿àÂç 5)­OTHERglc3FGL J1808.5-19522MS-GC01?áiBˆ©?ÖCc,%?Ý-{ÁÊî¯?ÖCc,%?Â7IbŸ‡o?Å.æÂJ=?ër-§X$?Å.æÂJ=?ÛMæËÚ?¶xØ$g?âYyŒš÷?¶xØ$g?¶iƒ|¹Él?±9!Èrb-?í2ϐv…B?±9!Èrb-?Û-łx?×3"}7?âri>Ãú?×3"}7?ˆlN"ÔD?­(2GQ®?ïžNžnC?­(2GQ®?Õ–†rS?¸–]‰yå?åvÿ´¼ÆÖ?¸–]‰yå?QûHJ?Z§ÖìàçU?ï÷rm}(?Z§ÖìàçU8MIXED4FGL J1810.3-1925e?ªÿ¸wRM¿¾(w~¢ÙpÀ7±C΋é®À9"y
2ª@‰Ä7@Š|Æ$<?À<"·Ÿ¿?ÒEkD¸Ã@¼«œÑ\@Öªß<;?ïë>bk]¿®w9>ÝW׿ÜèƒažÖo¿èPÄsa÷l¿ã#Îq»¿ïôU§ÒAOTHERspp3FGL J1810.1-1910HESS J1809-193?½Ùê›Ù~¦?ÇˊЏ5?ìD¬"Ð+?ÇˊЏ5?´?½zqØ?µG넦uÿ?íxPö+…?µG넦uÿ?ÖOú,	%÷?´.7#ÚZ?äØéûm?´.7#ÚZ?ÈsÂ~"I?«ÿ÷É/?éã`^ÿ.?«ÿ÷É/?²¦-È,'?ÅÀú"{ê©?í«:FÞòÐ?ÅÀú"{ê©?xu°OKiK?‡u­Çu‹?ïÏŸ8-Þ?‡u­Çu‹?Úb JÛ?¸yþ:+jª?âίڒvÿ?¸yþ:+jª?~£,4zQÉ?q/rmÕÎ?﹧ÅÆ?q/rmÕÎ"PSR4FGL J1811.5-1844?渥\Š3d¿¤lי¯iÀ8EŒîkóÀ9ã?¹SsE@+×IR"@ŽŽ¾tDu?Æ­'@
Üþ?Ý$)à¤&@ž¡aä÷f?ý	ø`Nt?ïû1~þá¿Ùv}_Ò"¢¿æ"ù2e-¿ê¶CŒ¿ïÿýF\I?ïÿ¨âaßnOTHERsppSNR G012.0-00.1?ÔÓñ&Ñم?Ô"ÒâTbG?å–l—>?Ô"ÒâTbG?¯Í8ò(À­?²Gy¬Jh‡?î,pÝsõ?²Gy¬Jh‡?Ù¦0qM?·VEC{â?ã,çõG?Z?·VEC{â?¶©[‹ï›? ¢=;¦"?í*ԟ©þí? ¢=;¦"?Ôê¥GD.¥?ÙOƯÚ×/?劭\]è­?ÙOƯÚ×/?t÷«ÎʅÏ?…	‡K	ÿã?ïÖ¨nɌ?…	‡K	ÿã?·kå¤Óí?¥Àè¤s?í#fâb?¥Àè¤s?Qó›|Íwï?HV¥ÒŒ…	?ï÷2ZVt?HV¥ÒŒ…	PSR4FGL J1813.1-1737e?ížñ•·•a?Åæ­ýÀ6…Fü=ÔÀ9OVcÉÔ@f€®¼š@T¾ÆyÌu?©$S…í?Ã@y—Ɔ@µKHÓ®h?öf¼ýÌÉó?ïÿ@OÁß¿Ò2l"¿¿âµƒž¿åéҁ—š;¿çEsÝGnT¿ß:md1'ÚOTHERspp3FGL J1814.1-1734cHESS J1813-178?°eÀ†|ã)?ÁøC',ì%?íóGï>"?ÁøC',ì%?¤®L)xc?©+Ô2˜?îµ=¦²:?©+Ô2˜?݆´Ä16ž?¶#ó¬ûå?á<¥çd±?¶#ó¬ûå?""h"oâ\?}l¹µÚÌ?ï[Ü»"z­?}l¹µÚÌ?»ýÒ¿Zk?Ä CÏ/?ì€E¼³?Ä CÏ/?rØx
€r
?ƒ)^/z]?ïÚO÷]´?ƒ)^/z]?ác¾š[?¶Oæj;$?Ý8ƒÂËIÈ?¶Oæj;$?;TÏ;š;|?0?"£úh•?ïü•fG÷T?0?"£úh•MIXED4FGL J1813.7-1536¿ã"®~5Ï?ðŽw&¨
À9rp·"@À:¥Mçê_…@ ^)dÓ@Í`ÛâêF?Åꐗ'X]?.77¸º?Ï8ÿ%­B@Òͺ³p?ì/8"9³¿Ý#÷p"¿éÿJ-J»æ¿âåPQQ+¿çB:73rô¿Þb'|,OTHERunk1RXS J181335.6-153600?ï
ÞÃwí?¨ÐÇúC?D+ž[?¨ÐÇúC?ï-͂¡§Ò?«¨bsã]¥?šFO´b¨?«¨bsã]¥?ì… ŸV®?ªûKIYT?»Öÿ£J?ªûKIYT?ï—E(J™N?r'$[þ#?Š.µû~?r'$[þ#?ê0·çÒ%–?þ@;ž*'?Ç= `·i¨?þ@;ž*'?êƵêÕn?ÈÎŒûÀD?Äç‰(TªI?ÈÎŒûÀD?ëšé(*Ê?°¶é
Ƭ?Á"[_T×Ñ?°¶é
Ƭ?ìîïþÄÛV?¦—k5ëå»?¸ˆ€ý>U?¦—k5ëå»AGN4FGL J1814.1-1710?äDñàhÇ%?Ç	j!†ã_À8ò(zrÀ9þªhö‹@ ~JL)@¹åi|?Ð23Xòà]?·åΑs?ñftù§ k@½®€0'î?Û$cAmހ?ìÔ_¾+Ÿ@¿æE^XûÅ¿ê)óÿk°}¿Û]"3¿ëBÇû¬´)OTHERsppSNR G013.5+00.2?é†óÿcw?Τ,¦Àã?Éä0sš#?Τ,¦Àã?íŠÜ"r7w?¹£ä(çˆm?³©ÜÜ7Ä?¹£ä(çˆm?ãu²Dò^"?¸øJ²‰]?Ù›vBÚ?¸øJ²‰]?îôÁmž&?+ޑVA? ³é&Í¡?+ޑVA?äå‹é
y?Ñ2æîGW?×à4è-ë?Ñ2æîGW?ã–Ó>‰†/?Ò2*Œ=?ØÒY'ìó£?Ò2*Œ=?ä)9E'&?Á\%‡pnŸ?×ÿ­tû³?Á\%‡pnŸ?çbf~(Ý?À´ÐÄJ"›?Ñ;3¯ÚE?À´ÐÄJ"›AGN4FGL J1816.2-1654c?ÊfW'¦¿ÁS|©É½yÀ8FñTk'À9Ñ×rB<»@Ô_¾+Ÿ@Ä[^Ëgr?ÏJ*,¤N?ê[éhÐú@-?ü¿ÒxˆQô?îê?¤Z¾¿Õ4Îÿ,¿åÀ ·/¬–¿îo/˜sÿ¬¿à± ‹ü"%¿ïþLké]&OTHERunk2FGL J1817.6-1651cPMN J1816-1649?ΪȜL¸?Ò¢MAÄÆ?èU}
ØìÒ?Ò¢MAÄÆ?¨Ïϳøc«?­Ÿªº/9Ÿ?îs—>v?­Ÿªº/9Ÿ?ٚÐ>
A?´à–OA™™?ã2¿àúà?´à–OA™™?¥•\|pç?"-Ã$?8D·a?"-Ã$?ÍÙ;>´4"?Õª‹¾S|?艱0RòÛ?Õª‹¾S|?t7x"4¸
?"nÈm6?ïבÌ°?"nÈm6?ÔÛþJÚU?¾9ó…?å'vڒÕ?¾9ó…?C£ÜüNÄÉ?DÕâõe©V?ïûÁUÜ?DÕâõe©V,PSR4FGL J1818.5-1656¿ž(Y·íœÅ¿ä¨ªxäî,À8×£Z»ÐÀ:^xèI*@ûÙc¯@÷‹7GN?ÆvÚèCuÌ?ٚcƒˆ
P@2 f<u?÷úÿåþÍ¿ïß4Bý«'?ïû>?*ã.¿à¸Gڊ%¿åz·\Ç+¿ìӋ,ïLT¿ïû¨LºÃ¶OTHERglcGLIMPSE C02?´&['ô?À¾û[‰P?í{4QÆ-?À¾û[‰P?¶Âr¯3¯'?¸Ô­õ¼È,?í'±©þ
.?¸Ô­õ¼È,?Ôcî‡1¸	?²ýÂÓ*³(?åμg#ü?²ýÂÓ*³(?Ç_P®ª^?§lp‹kI?ê(+ÔUhx?§lp‹kI?'¬o_ãX=?"‹-ñ'Å?ïµNB¥Žg?"‹-ñ'Å?}õs»ŠÄ?‰¤†,‹k‡?ïÅàäNÛ?‰¤†,‹k‡?³]j=`à? Ç‰ç«è?í"R¸3¸"? Ç‰ç«è?oð0/ÄÓ?s+=!qàZ?ïº@?'™D?s+=!qàZPSR4FGL J1818.6-1533¿îb;qáÖ¿RnóÞ)YÀ7^²²$«À9^[ÿÛ@"ú%u…h@;¾òïv?µ7ƒNÿl‡?ÒÿßÝ5¦@1í¿‹›ª@‰a´¥ä?ïÿõ4Ê㿽ë *F>¿çìÞ²þE¿éçÑ—Êâ¿ëŽ5Lèæß¿ïÿò~#¿OTHERspp3FGL J1818.7-1528SNR G015.4+00.1?ªãK"ïíY?¼g"¯l6,?îQËMµ"K?¼g"¯l6,?¢mOŸá˜r?¥¨¶°X·?îÙ+æy?¥¨¶°X·?Ð1-qõˆ?³ðÞ^v1?çç9iG<?³ðÞ^v1?šÖdçesZ?…
'•L?ï)LØ©W…?…
'•L?'jàË;»?´'"
ªí™?ïl¨ùo(h?´'"
ªí™?qòƒ;›xø?ŽømDë?ïÜù^-æ?ŽømDë?¸¡žåw­O?ª±¥îï?ìëÌ#Q
V?ª±¥îï?4/ŽEÐ??)'sÈ¿¡?ïýzcðë?)'sÈ¿¡PSR4FGL J1820.3-1009?²ù&oÞè·@zÿèƒÀ8òdtJÀ:®nƇ8n@x±Ü¤Û@^YåN£Ò?Ç=|!äI?ÒTÕd éo@KBôqW?ó	Gðjâ?ïÖ8ñ¹`¿É68¡1=¿äÛ
bY'l¿åépq'#[¿ê#u –
¿ïÿð懈öOTHERunkFK Ser?âºYþ#1?ÐJÁ]
¥©?ڋL¹ñ?ÐJÁ]
¥©?ÀûhmÉÿ_?À®*•?ëÁ%䍀(?À®*•?â¹a•=¶¼?µò«ìrþ|?ڍ<Մ'ˆ?µò«ìrþ|?ÈMu 4ö#?¬i›uÍó¥?é좷òÂw?¬i›uÍó¥?É?ìmë°?Ïê¬Ëid6?éºpä…?Ïê¬Ëid6?šFÇøm3?·°Ú°O?å	Y›?·°Ú°O?Ñ–S'Í¿?³U‡D»"?çt´Ö>™!?³U‡D»"?…ZSÀ¡?t[GÁ6û?殺³zB?t[GÁ6ûMIXED4FGL J1820.4-1609c¿é´HãYè:¿å^®óÀ7vÀ#jÀ9ªdÜ"«&@lúnp ý@RnÚ©.b?°Wá&öå?gêfß´»F?³£</±š@Ý<¥wÉ:¿Ý	üƒ×+¿çµv¿åªÒa6PÊ¿è{:3µ¿ë¿Ôj³w"òOTHERbinKleinmann star?Øl«è"A?Ò¢É*xF?ãÉùª½à?Ò¢É*xF?ï<e¼Gn?§îg"å7q?˜sH}ñh%?§îg"å7q?ãLEº¯M?µciÕpZ<?Ùgt‹ö¡e?µciÕpZ<?îᑰʖD?"–©lxã¼?¡æäïæÿ¿?"–©lxã¼?Ø`'»cv?Ñ¡åÐKSÞ?ãÏ¿l"NE?Ñ¡åÐKSÞ?ëÑà¿ÀAF?ÆCt=$à?À¸}þúê?ÆCt=$à?æ¯h¤ji<?µQõ¤FÅ?Ò¡.·+-‰?µQõ¤FÅ?èäEE·ù?»r®¢"¹?ÌoÆêé ?»r®¢"¹$MIXED4FGL J1821.1-1422¿à×3}'ju?™ÎWçG¢VÀ7"H¤´ÏÀ9Y{ÕctD@§i&à@M¢ÝåùÄ?¹Â|ò–‹?Æ®nþ:ƒ	@
ë€ìúi¾?óÒÑ=õ®î?»›Ð>ò.¿ä(@zi¿æ'ñ.«äö¿êAyHªi¿ëát#¾K¿á»]¤ YOTHERspp1FGL J1821.1-1425cSNR G016.7+00.1?¾Qe½
?ÊXí0O‡?ì5ÓH^_ÿ?ÊXí0O‡?·)ÌSÁx?¹H'èeߢ?íƑ±?¹H'èeߢ?ÙEøüÅQÈ?·A(k{p†?ã]W?·A(k{p†?Ä}ÑÁBî?§¯ÑSð*?êà‹¯yÅ?§¯ÑSð*?³ 'ìòËÔ?ÃØE܃#6?í›ûa¦†?ÃØE܃#6?}ø?û*?Š(Þ'
?ïÅà[?Š(Þ'
?Ñ°ŒÐq"?µyѬâJ?ç'¹¿Ç6?µyѬâJ?ne¦"WøÃ?`+Œ!>D°?ïášYˆŸ?`+Œ!>D°PSR4FGL J1821.4-1516¿îï
øÍAù¿Ý5%:ÍÀ8Iûçl‹DÀ9¢*9mÇ@Épgq(a@ŸGù"Õ4?ʹ~%õ²õ?áõ£àðEM@Bþ'Q@ïƒm2?ï½'"ƒ¸‡?˜hÀçCú¿è¢Ë§2ßP¿ëW*ß&Á‹¿î˜ìËoÕ¿ïÿA"VOTHERsppSNR G016.0-00.5?ÞAp><·Ò?ÕËãUݤ?àßGàá¤?ÕËãUݤ?¹çÝne?»—XGzú?ìÃ_ò?3?»—XGzú?Ûâ—îãfÜ?´t\Ð/	?â´ŽL'?´t\Ð/	?Éíq®ª3+?¬(ÜcYÔ?鄣"Us5?¬(ÜcYÔ?ÖVFö+k?ÔõÈo¬Ž?äÔ܄êyË?ÔõÈo¬Ž?'H%»'í0?ˆaøhh?ï¶ßhìä«?ˆaøhh?Å©/úµY?±ƒƒ%ã	?ꕴyÒª?±ƒƒ%ã	?{EtZ|?l&úk$ù?ïÉuÀLG?l&úk$ùPSR4FGL J1823.6-2345¿çÜ[ªÏÀ'ÛŸ'xÀ:&Mâ"sÀ;›mB"º?@Ã=¾Q‰à@;Û¾Ø?Îø¾'²!{?Ѓբ‰WW?ü'à@bMÖøtÆ?îøçþ¡f¿ç¼]éÀ#¿áä=Çᬿãù2±-4¿á_Cr¿ïø°ëŶXOTHERsppSNR G008.7-05.0?ï姀Wæ?i¹Ýb|?jXÐÊ"C?i¹Ýb|?ïsòS*?›ÂU7…v?Œ£=ͺ	[?›ÂU7…v?ïmǛàpÄ?Œ£»
Ì?'G':'?Œ£»
Ì?ï»v…ÃÏ?b¦ãͦÒ?"^¬å"?b¦ãͦÒ?ïƒîz؟z?'ù¾Vï#?aIØ!{?'ù¾Vï#?ì×s»¨Q?Ánìsþvà?¹Db#+kM?Ánìsþvà?ìëUÝha¤?¥=VÑâ¥?¸¥Q˜ÙÛ?¥=VÑâ¥?îQL	)/µ?–3ø!†¯Ô?ªë?iýh¯?–3ø!†¯ÔAGN4FGL J1824.1-1304?鶚wÔ¼Ÿ¿q™JÞ-näÀ8ÝäLESÀ9'ý÷Cõ@ÁªKÃwä@|5À¬-?Ëó²ª6ÊÂ?èh(=5ët@"£Ÿ¬Ù@i'|'v?ïøʁ˜ñÔ¿Þ1›cHNοç(¬âKº¿ïÿ¨âaßn?èÉâÂW}ë?åÙÑ,­ÝôOTHERsppSNR G018.1-00.1?à~[§­?֓teØw?ßÑÏH°§?֓teØw?ŜÎþçba?Í`ßW­ª·?ê˜Ì@F'h?Í`ßW­ª·?à"|"
O?µ°]–°œ?Þ×÷ëßb?µ°]–°œ?çÓ'n|,?Đb·ú˜?ÐYÂû#¨?Đb·ú˜?뛕êëú?ÎÁEº'6?Á'¨TP?ÎÁEº'6?uœâ1䂺?"(em"X?ïÔÆ;–·›?"(em"X?ß3îmöŒ?¹2š±™è?àfÉôº?¹2š±™è?°qç‡ýԛ?À"¤¥™àš?íñû=?À"¤¥™àšMIXED4FGL J1824.5-1351e?Ò0§"ÑU?¿Ý6syÀ6³"÷si"À9N?(3ü@#›Ÿ"X·Ò?û¬	sFHº?¤å¿b%??‹R·ƒ#?öŠÙv0@äÖ¼9ג?֋Ⱦâ(?â6*~®±¯¿Ú³8ÜÀ_׿ØcµÜñ22¿Ùsßà›¿ÌÚeçr~OTHERPWN3FGL J1824.5-1351eHESS J1825-137?à­›Ì~?ÓvòéI¸¹?Þ¥ÖÈgý?ÓvòéI¸¹?ë÷槥‡?ÇõŒFþIÐ?À eaiã…?ÇõŒFþIÐ?ä{R°F?µIye""®?×	ZäŸsÆ?µIye""®?éd—"[Â?½2
á|ԉ?Êm¡®÷Š?½2
á|ԉ?ç8xr`"]?ͦ*1èì?я?»F?ͦ*1èì?æX<"Ev?Ò"pjC?ÓO‡ºýu?Ò"pjC?èsl²–üÂ?¸Û(qۆñ?Î2M5¤ö?¸Û(qۆñ?áGĄÿ®¡?ÈPI|÷«?Ýpvö¢½?ÈPI|÷«AGN4FGL J1826.2-1450¿ØË«@"¢¿ô¦D¢Ç?ÅÀ6 a3÷À9i£bp7¡@ãR™€@J© öÍ?–\Û£)eT?¿gûfé2@ ¬B 6m@›6PtÀ¿ÖdΡ8Is¿ä ¹ÿȏ¿æ{4ßZÃñ¿è›Ù°
g¿ìwQ­Dq¿ØÇ¿Sg†OTHERHMB3FGL J1826.2-1450LS 5039?¿>éÛâzš?ÊÓa†­®¤?ì"ă°­?ÊÓa†­®¤?žïbÎ?¡á'>¡õ_?ïÇÈ£iÉ?¡á'>¡õ_?Þ¡(¯ ¿h?³Í°ÖI^?à¯k¨o L?³Í°ÖI^?–úðIõ.¥?€'UäÇÃ?ïH(}¢˜?€'UäÇÃ?¶£(j€?ÈTË£æz?í+šòxòŸ?ÈTË£æz?olõæV£?~ý|Ѻ'Õ?ïà"ì0•I?~ý|Ѻ'Õ?àŒE!Œ¡?¶&)ñLS?Þçu¼çô¾?¶&)ñLS?1šÍ9'Å?''mˆÀ?ïý̦ƒ¯D?''mˆÀMIXED4FGL J1828.0-1133?ÚOqèOµ¿ÂfS†ÑšÀ8Nµ‡5éÇÀ9îÐ_(""@&Þ÷q@ö¥†6æF?Ä/fÉû?âtöL"'@'5Ÿôým@eãmx(†?â ÀaŠ	?ԋ"|I&º¿Üi'ûr}¿êfs.ËÅ¿îrç;
¿ŸzSƒ4ÓFOTHERspp3FGL J1828.4-1121SNR G020.0-00.2?ÇñÈ&AU?·éݘÊ?ê=öo«?·éݘÊ?ªxL~õÀ?¬rcëNýp?îX{8nD?¬rcëNýp?ÏÀs¬œ?³&¬¢·…?èúãÔÙ?³&¬¢·…?º¨ÁP~ö?›‹¡{"³Ì?ìªçÕð?¡?›‹¡{"³Ì?´P*Š62?Îí…È	!D?íuú®þn?Îí…È	!D?un»s…?ƒÏô"ð?ïÕ"üPÀY?ƒÏô"ð?šÊW°È?©X@˜Rp?ï)­B:Y?©X@˜Rp?g×àHùó?T:™b°@?ïèà(@³F?T:™b°@PSR4FGL J1829.4-1256?ïë¨Ó{ñ¿ñeªIFÀ9cQ³PúÄÀ;ƒ:=°@¼]¸ÂÔ¦@"¯ûî|?ÍÛ`#`"?ïÛ}i¸*~@õo›Ìz@³ɝÃJ?ïƒ{_œÈ£?ïÚËB‰Œ?ˆ¢õ¸ÔG¿è¹"8à¿ïþ>>ª	Ô?ï¨wÆOOTHERspp3FGL J1829.7-1304SNR G018.9-01.1?ÆC =͕õ?Æk:¸°²?êoðŒšƒ?Æk:¸°²?«ôÕ¦ü]Ó?¯=^÷…}Æ?î@²¥Y@c?¯=^÷…}Æ?Ò;¸Žˆ%?°¯RÜyp¸?æâ#¸¹;î?°¯RÜyp¸?Ÿ6>…•¹b?‹&VŸ×Í?ïN·ÕU?‹&VŸ×Í?‹‡ÖÉ[ñF?§'2»ƒ?ï'à¤èN«?§'2»ƒ?wS36ÃËn?…DÊ.?ïÑY™¤Va?…DÊ.?§ÿ¾dÔ?•3èf•ª?'o?•3èf•ª?[ä–èÆDÌ?RöŸöIž?ïò
´§½?RöŸöIžPSR4FGL J1829.5+4845¿Ñ³.Áž@7Š\å´$À8¾©@'À;ûl'à±@B˜*Þ@ÙuòËd?¡òœ*'?¯'öiÿ"5@êeÀN9@ë財*¿ÄI'C¼˜¿âßwßµ‡·¿ç›˜w[¿ã".ülοë€JœÜD¿ÞU3ÃÑÑnOTHERcss3FGL J1829.6+48443C 380?ïȓñJ@Ò?°Ý¡vÖÍ·?{¶wbÏ?°Ý¡vÖÍ·?ïð‰]"ä1?c³ :&?^íDe"o?c³ :&?茶`^¡?ˆ€«4l[W?†=nǏÊ?ˆ€«4l[W?ïéãâÅ\?SØHÑ·	š?fÓ\¬Q?SØHÑ·	š?ï÷mJú¶?Lšž°'ë'?Q%ÅT
~?Lšž°'ë'?ï¾'±'ˆc?…¯,Ë1Ž?€v²®KT?…¯,Ë1Ž?ï˜7¥xÒ?ŠGŠ}þÑ?‰ò¸r/š?ŠGŠ}þÑ?שׁ~ õÌ?v€$»û?"Õ`~¡Ä×?v€$»ûAGN4FGL J1830.2-1005¿ìصú.&?«W2"Ç{À7×)ž^û8À9""išÎ@¢ÌÉè>@
Å㤀?ÄA¼bò= ?Ûæ€<¦N‰@ÓÖ¿•?ôÈ[á¨&$?ï±½¢bk¿ßZ¿žæàt¿è˜8p‰Õ׿옝?ìT'¿ç?Ô@ßn:¿ïÿ·ÀÌ
ŠOTHERspp1FGL J1829.6-1006cSNR G021.5-00.1?¿Ÿwî¾?Ë¿ÓR€‰?ì<ì(?Ë¿ÓR€‰?¤žN |+?§°âóº(?Þþ~?§°âóº(?Ü8@{ù©,?´Áõìk?áãßÂ+j?´Áõìk?Ÿš" € ?ˆ_¿¢õ?ï+ß_?ˆ_¿¢õ?Ñø±pë?ÔݯÖûW'?çyüƒ§G‹?ÔݯÖûW'?șÍ6çŒ?ƒ.ƒ·PE?ïØf²LÕ?ƒ.ƒ·PE?ÚZ•Ü?¸3õïPa?âðÿRõµ?¸3õïPa?8b>-ù³?0¡çK@Ð?ïüó¸æ?0¡çK@ÐPSR4FGL J1831.8-1503?¥Ô"HJ<QÀÈõÝgNÄÀ:™ °åºÀ<RG—nF/@ÐõLrÊM@Ê}Å'¼Ý?Õ8¥ƒ1Î.?ïý'ÒÕûJ@ÃC·õf?ü€Ó6ô2í¿µL+@V?ê?ýkûý?ä`s^™¿åª%mwҟ¿ï$X*Ž¿½pc×%ÁOTHERsppSNR G017.4-02.3?åJ²gŠ—?Ë`mÅo?Õj›0êÐæ?Ë`mÅo?ÍbTF[â‡?ƚ¡Rïf?è§jîi^?ƚ¡Rïf?éÀdmF?¬q0JÉÈy?ÈþoÒJæ?¬q0JÉÈy?ÅäXüèÀÁ?°hÖ9½Mï?ê†éÀÅÏÐ?°hÖ9½Mï?Ð~97?m?ÊÎY%~?çÀãd`I8?ÊÎY%~?ž*õbrZ?­B™Iëñ?ï¨9o?­B™Iëñ?ßQ.ƒî?À,7î{?´?às×yè¾	?À,7î{?´?¡£ŽÒû–ã?–+ÁT²×?îåǴɲ?–+ÁT²×	MIXED4FGL J1832.3-1433?à™Ñ'¯D§À¼,†pÇéÀ9ÌEŠMÌ<À;=5¾(@]l²ŒÛ?ÿSýÈîû?ЉCá`x?ÙmR=åhÐ@ø£ë,3@À<-'Å¿ïxvétù?ì®ç¸5f?ÒP×Þά÷¿çŽáDS(¿á4&¾Ýà¿ï÷åê«%OTHERsppSNR G017.8-02.6?ï¦á(#ŠŸ?Üe}$œV?†Gµì΄d?Üe}$œV?ìÙ(¬¶E¼?¿'¢X?¹6º˜(¦?¿'¢X?ì&º¦7?¥Ó>ސƒ@?¾Éë'*ÎF?¥Ó>ސƒ@?î†V½°?'%-ÉØJ?®·Ÿ
'Ú?'%-ÉØJ?ìªóôë?´ô{Œ®ù?º¯Ïˆ`X¨?´ô{Œ®ù?äÑ0'Þ¦?Ñ'Øó1ø?Ö]žÄÚBµ?Ñ'Øó1ø?çjëEUA?²Ý†Þâì!?Ñ*)uU}Ç?²Ý†Þâì!?èQGì[f?´,!>Ó 2?κàN'gÕ?´,!>Ó 2AGN4FGL J1832.9-0913¿éì'£lg¿ÁÁ›o¨ÚÀ8Ó^R›®GÀ:†••þÚf@h'Ô±Ã@û]‰H¾?Ìwt«£‡Y?å·Y}ʱ@Q['—@¶HW²™p¿ã€üŸxUÒ¿×xû~æåÓ¿Ôîÿ&¼,l¿çXUÌ»/¿î–÷'ê)Õ¿ïë;³´MOTHERsppSNR G022.7-00.2?¾îH¡É,É?Ò~…ŸšB?ì"6ëÆÚg?Ò~…ŸšB?¾÷í.c?ÀZ›æìo?ì!Z3Ž^?ÀZ›æìo?ÒÐ#—<z¸?±J§öÏ?æ—î4a¤?±J§öÏ?Ò2¢Îf?°5?߶Uß?ææ®õ˜ÀM?°5?߶Uß?"4Š—þ? `Gý¼ü?ïf_ãóãp? `Gý¼ü?ƒxl‹4C?'õ' 2.?ï²MüjÓ?'õ' 2.?²ú*ü?£|%l*ˆ…?í ¾ýè^à?£|%l*ˆ…?Ë.3'tT?8˜S±ý?ïy¦Žct]?8˜S±ýPSR4FGL J1834.1-0706e?ìâ
?âºíÜçÍÀ7‡†Nc:bÀ9÷‡©­
@ ºÓ»ÔW@B¤¸±?ª6CM1·?´¯Ï;#@½M%LÀ£?þ8r_˜ìË¿ï}1NV¥(?ïO¼5¥Ô:¿Ø_~Øտܳ@S'D¿ä…|áÒîO¿ä˜…2ˆKOTHERSNR3FGL J1833.9-0711SNR G024.7+00.6?â^zuME>?ÒÞ]o'‰?ÛCeuƒ?ÒÞ]o'‰?ÛL¥¨¤,?ÏÊ3ÀKßý?âsY­+­ê?ÏÊ3ÀKßý?á²ÿ#êž?·ä›]…?Ýƚ¸*Ã?·ä›]…?â'õÎ?¹GAì>?ÚÝ÷Èàc?¹GAì>?ÙcŒC'q?Òsû…	 ?ãN9Þ6ñH?Òsû…	 ?¾Ç"ß½·¨?Ä#ðcï's?ì'
"I?Ä#ðcï's?åPÁR_?¾µŒ,?ÕÙ^}[Aç?¾µŒ,?ÁþãÞ{?´™¶1ñ7è?ë€~‡a<?´™¶1ñ7èMIXED4FGL J1834.5-0846e¿ÖÞ˜•/¿ÑêÛá<ÆZÀ6øêúÀ9´ëvÛÿp@!q3­ª@øã["‹?©ãZ> 2a?¡7ßÀD~4?ö˜ÏTf‰¢?ðX#…@FA?ê!j³Ó¿×AIÌR¿Þ|cÓº¿ßü
1¿åèå1G ©¿Ö¿²ÝãJ"OTHERspp3FGL J1834.5-0841W 41?Õ`<‡š¿?Ôº2B"Ço?åOôa¼2¡?Ôº2B"Ço?Øê	~Xöf?ÑşUŠü?ãŠû@ӄÍ?ÑşUŠü?âN¥ï,?´›‡©ñÅD?ÛéÛb´!¨?´›‡©ñÅD?Í~:/H9w?¾ôl}?è qt-ñ¢?¾ôl}?×ÀIì³"?Ôlý
]?äÛ	¦qï?Ôlý
]?º]H…Ü?Ãùkç.ÍÉ?ì¼TVïP?Ãùkç.ÍÉ?æ‹ûžœbÍ?»&½w!þ
?ÒèÂÇ:g?»&½w!þ
?¡w¯ÜH/?›@"5=?îè…;w-?›@"5=MIXED4FGL J1835.7-3258?"QìÙH
zÀ&¼q'êRðÀ:"¾@BÀ<#=,±8ó@³7ƒ$O@Ê#9Àëî?À‹ön?×ÍýNtØ@R° ě¦@J~}"N?ïÿ?`h¤¿Ã—Ëù")h¿ãmß âM½¿äQQ¿î;Äf̽³¿ïûç6Û^`OTHERglc3FGL J1835.7-3258NGC 6652?ÙªŠŠ)†"?ÐÎÍÃlѺ?ã*ººë<¾?ÐÎÍÃlѺ?Ú®cøo_?ÎÛF§˜¾?âò¨ÎÈP?ÎÛF§˜¾?ÛTƌ§ÿÊ?´sJºäB	?âUœ¹¬?´sJºäB	?â3x¾`V
?°úzþˆc?ۙƒ?Sí?°úzþˆc?¼.­žÖ'?ÁÃÞï‡?ìz=ÊL%.?ÁÃÞï‡?°\ØÚ j±?¾¸#6T¿?íôdä¹±?¾¸#6T¿?¹ñ!íoí?§"N¢d\?ìÝaÛùKÂ?§"N¢d\?µy4jÐ? B-"_c€?íPÙrˆÄÆ? B-"_c€MIXED4FGL J1836.1+1143¿äSkî¡Äò@!\^Ô¡­dÀ:uOøÃÌÀ;ôWVP@Iބ…5_@Úµ€í ?Í°£vg:?Ð#Ëâ5!@­Ácâþ?út"« «¿ë¥C¡?€I?ïôἩi¿ÝCm¨z-¿çrº'Gm}¿Ý‰šÈïÿð ¼x—OTHERunk87GB 183342.2+114143?ïzâظún?çúw@X?£¤î3?çúw@X?è/$f€?Éâæů¢?ÏCóneýû?Éâæů¢?îù&,?'Ú'Àä	 ? n'*/a>?'Ú'Àä	 ?퐫°ÍÌ?–t½}_¸^?³z¢3l?–t½}_¸^?ìxeøŠôC?¶—|üà?¼<Ð;¨]é?¶—|üà?ÐýÖS΁?оZ1ˆI?çüÖÀ?оZ1ˆI?é]z'Ê?µ-bH?˾‹®ôÖ?µ-bH?àV%îüød?¼NÙ[?Z£?ßS´"9?¼NÙ[?Z£MIXED4FGL J1836.5-0651e?ïÿúr]¦µ?ÄCO¢ÝÀ6A‹sf)*À9"Â(.s@!&¤†‡™@;ÌDÑ	?›2Gk'í?Œ8e!Aï?ñ8^€¾×A@9nY$¿áµþŸWɖ¿–¦…Üàc¿àÔ*ÄϨI¿áÖG4q÷"¿âÃai&Š¿ØuØstOTHERpwn3FGL J1836.5-0655eHESS J1837-069?ØQ¹Ý.?ÓuÇáð9R?ã×#ti?ÓuÇáð9R?ìmä­û6©?ÅcÙʝXÒ?¼Ú&Jº?ÅcÙʝXÒ?âÙ݉d¡?µùŒêÑÈõ?ÚLEòí6¾?µùŒêÑÈõ?çãAAOð?ÁvŽÞ
É?Ð9}}aÞ?ÁvŽÞ
É?ßíDË?ÓFà‡K]?à	]ÿ1w?ÓFà‡K]?æ-EµÛˆ?ѯØõÒ?Ó¥Ït"Hï?ѯØõÒ?æÒlYš{?½^<Ýg?Ò[á'LË
?½^<Ýg?Û䘇*M?Èvƒps–·?â
³¼|êÚ?Èvƒps–·MIXED4FGL J1836.8-0727?ìF6ߞO¿Æ¡)ÛƏÇÀ83È-*ÛvÀ9õ}å-@¥ˆáe‹@8ƒŸ\Q:?ĆÒíx=ÿ?ÞYG™ò"í@I[»èxû?õŒ>Ù.°¿Þ†=0âöÛ?ájÅÁ?Ðпáµ'ÿùJ¿ê½®ˆ*Ü¿ëleöÕ¿ïÿð°×£ÀOTHERunk0FGL J1836.1-0727NVSS J183652-072453?¿‰œvmŀ?ȝ÷—{²(?ìÌq2GP?ȝ÷—{²(? _ÿ':?¢Ìcˆ?îú.-Ëü?¢Ìcˆ?ÊyÌTân?±òfÔ²?éaŒê߇e?±òfÔ²?'dۜªb?wx"5ƒ>i?lŸKÆ?wx"5ƒ>i?¬š/'/k?Ë%T7埂?î6_Üù.™?Ë%T7埂?r
¸¢i¾?^"GÅæ?ïÛꎡ|?^"GÅæ?˜‡¬r"f?Œ†'Ý3?ï;œOßð?Œ†'Ý3?'äcšHÑ?].÷ŠîÛ?ïþ¹>ˆ?].÷ŠîÛPSR4FGL J1837.6-2904?âKý¼PJ=À$"¹,HÀ: š=-‡ùÀ;ÞËêN½Ó@¢Câ-@Qš&‡S?ÌÇ`|B?ÝÙoØ2@4f'ëØ+@	…nVŸÉß?âó\²¿Þ¼l—ØÏ:¿äJ½"s嫿薣L;¿ã%žÀJ‹¿ïÿ-<y-OTHERNOVV5668 Sgr?î³ËØõ¾Í?¬kJr´Þ?¤ÃBt¯'?¬kJr´Þ?ì¯2*¨'Ú?º´àÇ.?º†nª¾Á-?º´àÇ.?êûnoì™h?«Éê¾Q?ÄF@Mš_?«Éê¾Q?í–qÕk"?–&ÇüÈ?³LqVÉ)C?–&ÇüÈ?í×>ªï¥?´æÒ+WM?±FsvZ?´æÒ+WM?ÙZB@c¯?Ò¼•µ¼îf?ãRÞñßÎ)?Ò¼•µ¼îf?çÄÜs2ýƒ?²ÐW"–ë#?ÐvGšù?²ÐW"–ë#?Ù·›—?»¹Ì~/Ó?ã$v2r5?»¹Ì~/ÓMIXED4FGL J1838.3-2148?êÂú¥fñÀ‹;26À:h Ä0FÀ;딾h…û@Tñ¡˜kœ?ûžƒ
f?×µ˜ñ/?îªâ+Ù¢ž@&ó|cþ­?óZ…tɀ'¿éK—¾":?ïÝIúÑÿå#flE£x¿Ù££Þ–ú¿åñ0ߛÜj¿ïâÁáaYaOTHERunk1RXS J183818.2-214857?ÍÊùŽ?»q\c®%B?¦ã ¼²$?»q\c®%B?ߪ®ð}?ϚÉfÞ'à?à*¨‡óÿÂ?ϚÉfÞ'à?ìŒ0°ªŠá?¤bϵ¸È¯?»žzz«¨÷?¤bϵ¸È¯?ß5²Sú¨þ?·Ï¼–ª?àe&Ö«?·Ï¼–ª?ìÔ»rv-ó?ÁOqbø?¹Z$ntQá?ÁOqbø?¼Ü[ ­?Âì~ImBŠ?ìdt‹î
_?Âì~ImBŠ?鏕';a´?±išq‡Œ?ÉÁ©÷y2?±išq‡Œ?ÁBøɼi?°xQ›Ù.?ë¯A͐þ&?°xQ›Ù.MIXED4FGL J1838.9-0704e?ïÜDU‰8<¿Ý¿í@_Á‡À7c½ZiÀ:
²p*4‡@"EÑ4O?ýTç4?ª­ƒö?ž%.§w§?õ-ÑD*Ò<@SÖK¦¿äWLíï\D?ìÛÊ`áÂ'¿Òé,êCÖ¿ß4<Kµ¶¿ÜÔ–j:¿Î¿r[½OTHERpwn3FGL J1838.9-0646HESS J1837-069?ëڌ1m5?Ç3
÷ÞQ?À•Ïë:K*?Ç3
÷ÞQ?îžzÅK¬¯?±4ùI\?¦S¨±€?±4ùI\?åÐaœ?·ync²m?Õî_Ý=æÉ?·ync²m?îfµŒûaÇ?ž#žâ&þ?©"§-¶.–?ž#žâ&þ?éÝC}_+?Å0§11Ñ?ȊòöƒU?Å0§11Ñ?êQ7uë%?ȑ fgh?Æ»"(Q‹l?ȑ fgh?èÖTx?¸¹×Ók@y?Ìñ¦­Ë¢"?¸¹×Ók@y?ë5qáU?·Z.ûý";?Ã*8z«ÿ?·Z.ûý";AGN4FGL J1839.4-0553?צ$N`W¦¿›8g®´À7Eõ­–§À9T'œýÒ(@c;'PŸÖ@Ð:?–îÄ?¯RSÈ)$?ՖBÚ¶@(dÀ
¡©@Ë#œè-¦¿ØœOAÙ´?¢b`¿ªÇ·¿áÈÖ"‹ñ¿å¼žK°»¿ì'ê@%4¿ïÿôým~‰OTHERunk3FGL J1839.3-0552NVSS J183922-055321?"R¾nd?«!u«͋?﮵'ÍP?«!u«͋?•{ІÈý?šÕYŠÌ&~?ïT!NH?šÕYŠÌ&~?¯E'*kaÄ?¢>~šÎ?î¦Ý'…4?¢>~šÎ?r$ß$Á•?i¤pð…‡?ïÛ¶Ašÿö?i¤pð…‡?†îí^Ù?³SWX?ï¤DJ‡¸œ?³SWX?hIup…Ô?wI¥4µBÝ?ïç¶r˜Mê?wI¥4µBÝ?«Âþ]Ø<?£—ZÚTp?îCÞ "|?£—ZÚTp>ë\%_ùˆ>í\F÷¾Ñ?ïÿä£ûi»>í\F÷¾ÑPSR4FGL J1840.0-0341¿ïêIò‰Â.?ëXéÀ9iS$jB"À;?Ú˓é@ŸAЄè2@Š…) ?ÌÖßuEý:?êù¬ÿ§ël@Œý©äj@'bˆ‹T\¿Öüz$r뿧Š
¿Ó‹‰ þé¿å»;u!M¿ïúøÞ£¿ïÍQ!ZÛOTHERspp2FGL J1839.7-0334cSNR G028.8+01.5?µ)ò€†:Q?·³Qsª?íZÁ¯¸>ö?·³Qsª?µÂìhRã?¸xî0þ-K?íG½Â©ïc?¸xî0þ-K?Ԕ›¦lÄW?± ÞÀè
?åµ²,ɝÔ?± ÞÀè
?½¯	å©_? BÖÒ$ɐ?ìLJÃJÔ? BÖÒ$ɐ?k¬ Ãvç?knqI±¶Y?ïäSëÔ=É?knqI±¶Y?}äÿ–Ÿ#|?‹ASaAˆ?ïÄ6Ô!'?‹ASaAˆ?¥{%ÏÃ-Y?'ê+/î*?î¨M£:Æê?'ê+/î*?yï
¹ë<?eÖ$"j×C?ïÍî!¨"ª?eÖ$"j×CPSR4FGL J1840.0-0411¿íÍ
Ãü³^?ã²â`1îåÀ8Ë6Z/ À:¯X¶zzð@§qºGº@Â…îÁê?ÀéÁЈg?ÕTpšœÏ@T´:ç?û£gΛY¿ëDä þè©?îAÔKFOp¿Öç¨ñ%r¿äd˜0
¿ìÿ"=ßßy¿æ°Ë¡ÖªOTHERspp3FGL J1840.1-0412SNR G027.8+00.6?µ¡fK÷@?¶¡C+)ͤ?í_+Ó(¨?¶¡C+)ͤ?·¹¬-3ِ?¹r	,ýŸ?íÊz̞?¹r	,ýŸ?ÓÕT]•Õ?²†ê5c?æU±Q5?²†ê5c?Ȓó5ùH?§¬D»«o?éÛC2¸A®?§¬D»«o?yxÕ×wË?|;xÌÑr?ïÍÚ,u™?|;xÌÑr?€ä"í§?Ž4Çß"?ï¼o¡ÅÚb?Ž4Çß"?®™*r•)æ?Ÿ{"dÀ7Ø?îmY
§!?Ÿ{"dÀ7Ø?†·cÍ2@?x@+™¬Óú?ï¥"siÑw?x@+™¬ÓúPSR4FGL J1840.8-0453e¿ã܈.b>?¿¹Ÿ'À7Y…tH§9À9'$~d@ˆ¾)pçŸ@úh±šA_?³uÏ:p`?Ð4°@¥¾@	G{À?ütXåIpa?îfKŽs˪¿ËOøæ±${¿áç—Sn¿çá}ÿ	_û¿é¹Ù«¡¿áĖgµñ¿OTHERspp2FGL J1841.2-0459cKes 73?žã5KI&?³wN§¬!Ÿ?ïç~:(×?³wN§¬!Ÿ?£'Ï<Ìa?¥êš2Þ´?îÆî"Õ9z?¥êš2Þ´?ÒãÆ~TÜ?µp>Ó
ºª?æŽÀÕó'?µp>Ó
ºª?¥}o–‹©3?ŠÊïØ¢ã?î¨)‰†ý?ŠÊïØ¢ã?‰òš'Eì©?³tÑÛäɗ?ï˜5•Ûkn?³tÑÛäɗ?t´¼V{@w?ƒÊ¿«LŠ?ï֖‡–a×?ƒÊ¿«LŠ?À=ëLXŒù?­d¥@øµâ?ëð…,éÜÂ?­d¥@øµâ?L€¡]M?>/ùëHé7?ïøßü:´Ã?>/ùëHé7PSR4FGL J1840.9-0532e¿·@|ûÊ¿Éc\ɯŒÀ6ÁHO$*'À9¢ö{@!À¤¿:¾?ÿžá¢FçE?¢qNCQZÞ?~¢¨¿"?Þóå÷1?þ8=ägF?çÞ&'dA¿¹j"Þ|L­¿ÛO
*á¿ààÙÿ»6¢¿ãäkß÷÷É¿ÓKA\k»»OTHERPWN3FGL J1840.9-0532eHESS J1841-055?Ôñx›i ?ҋ¢Q>ƒ?å‡9C²K0?ҋ¢Q>ƒ?ìN<华?Ç*pìÏ?½Žèӓ?Ç*pìÏ?âÓRF±¦?µ$d¨}
?ÚY[ïrœ³?µ$d¨}
?æ'¬—M9?Ã
2Å
qÚ?ÓÓ°¦ÑeŽ?Ã
2Å
qÚ?àËG\—A?ҙ'ò	??Þiq÷FÑ~?ҙ'ò	??çN¦Œ-?ÑYƒâÖ¬þ?Ñcóزç§?ÑYƒâÖ¬þ?ç4Q/6h?ºþ}Z/º?Ñח]¡"0?ºþ}Z/º?Ùõkß
?Æô/ʃ?ã~Jwû?Æô/ʃMIXED4FGL J1842.2-0751?ï(R¿•²¿ø֍
?#À9m‹U38<À:í‹ÿ}#@an"B€@]™`Ž¶?ÐL]їb?Öļµ'•?ý*áU
È?û¢£h¥Zî¿ïúHÿÏ?ïÏف¼O¿»³¦
@JÉ¿åÛêaˆ0;¿ìXG¢'v¿ÇF£¨f;OTHERsppSNR G025.1-02.3?ëÛZÀQ$œ?¾8KËÛ`8?À'"þ»m?¾8KËÛ`8?äOÒõ(G?˃(ðJf'?×`ZÓ¯s?˃(ðJf'?åä¥ï	Û?±ü¶ž<`?Ô7ú´!ìJ?±ü¶ž<`?ç+''¿4ß?±+g*ê6?ѨÚځ–C?±+g*ê6?҃9ûú6è?Èì!x~J?æ¾cäŒ?Èì!x~J?˃Q âH?ÍÈŒ½Ï??é+·Ç_®?ÍÈŒ½Ï??ÜÍÙ½ 1y?¸A'÷õâž?á™!oçD?¸A'÷õâž?˝'ûP ‡?µ˜2ñïÆø?éŸA+÷Þ?µ˜2ñïÆø	MIXED4FGL J1842.5-0359c¿ïÚ¢ÄPâ?Ãå>]³ºWÀ8
°Úþ¾·À9Ÿ»	Uê@Ýp3Ü@jZaueÞ?ÄèÀHZå?؅ZZna@\äŒ×ê@‰Ö€TÏ?åi¹×ý'w¿á<Ó$Õ¢^¿å€™¸£J¿ê?*b{ö¿ïþmž"ÿQ?ït4à‡iÁOTHERunk3FGL J1843.0-0359cNVSS J184240-035858?à½	ô†¶?Õeöæ.?ޅßìò"?Õeöæ.?ÀhÄsž?Áç;ÐÅ;?ëåúŽãz?Áç;ÐÅ;?ٖˆ"Ûç?µz8ªoP?ã4»µ'v?µz8ªoP?Ö!K•»Ï¶?¶ll²•Dô?äïZ5"%?¶ll²•Dô?Ô©"0ã'?֌xd¯q?å«|¶gŽ7?֌xd¯q?{ØéÕ·þ?‰xØÞòÌã?ïÈN,!µÌ?‰xØÞòÌã?¶óԕÇf¬?¥HÂÜY?í!…m+–K?¥HÂÜY?/5ϧ?vӅ–áè?ï»C("êœ?vӅ–áè<MIXED4FGL J1844.4-0306¿Ý‹ù÷
9?À0¸@¸À7±Ÿ°4ÒÀ9zh»«<Y@KŸÅÒ=@K9âyÝ<?¼@|ÇÑ»I?ԗ?a¿¸'@7?tN†@k%ПX?ï%)œ±|¿â0öýø¾Ã¿å'0^—ÿ¿ê–—†™ã¿íïßáÒmv¿ïöÁ'ÜæöOTHERunk1FGL J1844.3-0309cNVSS J184431-030716?T‰«K.?¥ìåT¯¹ÿ?ïÝ[÷]Ö?¥ìåT¯¹ÿ? ³Û-E…?£¬MðX?îôÂLô­ð?£¬MðX?ÁYð"Û¢[?®¹)"¿cY?멃ÚÉi?®¹)"¿cY?›Ô~Çy?‡Jóùv?ï!\ÚÊx?‡Jóùv?xñ4<ÿ?©6¯?ïΗ•ˆh?©6¯?r;Ϩë?€÷£'žgÒ?ïۉæ?±é?€÷£'žgÒ?¡žkPá
?™èZñ'?îïFø/?™èZñ'?2GùÓeú"?'žŸ|ëö1?ïý·îΑ?'žŸ|ëö1PSR4FGL J1845.8-0831?í"c)›ýÀH㞠jÀ9ƒºéuzÀ;RALÑiê@#ï{M~@©"˜€•?Á"©…JV?Öå-a4l@PÔ~qõç@û†°ð?ïöׂˆ[¿â±Âëc'¿Ýt^ÁVw¿åÞ¯îo´Ä¿êîU'ÙŒ¿ïú–ŸVOTHERspp1FGL J1846.0-0831SNR G025.1-02.3?Í0!Îå^r?Äöç'–ó?è³÷ŒF¨d?Äöç'–ó?Ö¥½C@
?ÇÊX¶ý¯?ä­!~Þ_û?ÇÊX¶ý¯?ä 5j%?³ÑݑlÙ°?×Ô¿•+˶?³ÑݑlÙ°?æï€vÕ?¥Ú¶;¬?Ò!ûÎÿU?¥Ú¶;¬?£ˆ<³'FÍ?£yÑB6]?îÇ|4°C?£yÑB6]?¢±àΑ'?¬\+lBÝñ?î×á¼'?¬\+lBÝñ?Á"¶^SûÞ?¯ïv¥5ʋ?ë›hk?¯ïv¥5ʋ?Èé2ÜÔµW?ª/¯;´~?éųHÊÒª?ª/¯;´~MIXED4FGL J1846.9-0227?ØLÎ/d¿½
ò[ýËÀ8ï͂Õ2À9¥rE—¹Æ@BAê04ü@R+Ù¢ž%?ÁƑIhÿž?Ó'mb*W@Á"tŸ@ŠÒÒË?¬ÄÉ¿Òu`Õ,î¿Ú-³Âd¾ñ¿èëð«Ï¿ëîÈáÉ¿ëW€OE¸qOTHERunk1FGL J1846.8-0233cTXS 1844-025?¹tY.1¦?ÆﱆÓÍ?ìÑtÚG‰¬?ÆﱆÓÍ?­n±î·ô?¯œ7è%x?î)á/ý–?¯œ7è%x?Ê8ñ"kÌ?°ï;þ#÷?éqûšå
?°ï;þ#÷?»_<•Kp?£GJ(ƒ†ý?ì"mV'ÿ?£GJ(ƒ†ý?¦Bed»€?ÇO€ï‡?'?î›Ù¯€®?ÇO€ï‡?'?x|rZ#+»?…Àzob‹?ïÏÁ?…Àzob‹?•…Õ'ÙÇ?‰AcB¾˜?ïSÑSÍ»?‰AcB¾˜?c®Ôü]"t?W÷¶g~?ïìQ+/k?W÷¶g~PSR4FGL J1848.6-0202c?éø(¨E€¿ÔQlĤ_EÀ8RW˜mI¯À9¤mvûßà@ôüî@ç¶ãV|?Êk¿m"¬?ל;À•G@TUêî @z˜v. ¿íœ"N‰{?ï-ÇW嚿Ú<ßï¿@¿êh{œ"÷¿é5BEî¿ïÿ*±0OTHERunkNVSS J184840-020408?×°äRÇ?Óò½SÕa"?ä'öÖ¿?Óò½SÕa"?µÜRKE[{?¸'¨®r_<?íDu¶nA?¸'¨®r_<?Õ¸¸Cäíf?´©2s,¸ê?å#£Þ
‰M?´©2s,¸ê?̲œAa¼?±ó©h®:?èÓX狀'?±ó©h®:?É[ÈéîÏ?Ó͊©'`?é©
ùE"L?Ó͊©'`?}Ob¹<²ó?‰Ô¯ÍÁ?ïÅa:¤ãò?‰Ô¯ÍÁ?¹ýZãj6ï?©K~Õ.Vf?ìÀT£'¹"?©K~Õ.Vf?yZØ@+ë?pæõ§ÀXŠ?ïÍÙJ<AØ?pæõ§ÀXŠ<PSR4FGL J1848.7-0129?ïÅP«'é￸}P·
HÀ8'ØÚø	À:S‰X@úFô±e@ND¬{?½©O€W–?á1Ú£O%@"]Ç5ï¦?ûøýlÒ¼%¿Þ›C<뙿ÛwŒ>] ¿ÓQGpĎ¿âgšþôgF¿ïü¸Lã¢?æ®&ïXOTHERglc0FGL J1848.6-0138GLIMPSE C01?'sŠR?µüû$	[?ïlg?\êÅ?µüû$	[?šI,®Y¦,? "½ø§#Î?ï-¶šc÷? "½ø§#Î?´›V\Ró4?¤ì±s«?íl•4Z$º?¤ì±s«?‡-Å0m?yDƒ¹oº-?ï£ÓH´F;?yDƒ¹oº-?%ˆ4tŠ?»Ãå¦0œ?ï~Ó¿§—«?»Ãå¦0œ?lÅۑ§Þ?y×?·?ïã:$>"Ð?y×?·?'êADw{?…¿]'F,ú?ïp­õú¡$?…¿]'F,ú?·—žË,?+Çüî=ÿ?ïÿbCʍ¶?+Çüî=ÿPSR4FGL J1849.4-0056?ìڊLl¹?'|[p>+ŠÀ7€3)'°À9¥€(¯K³@£‰™o@-"œ)–Ò?® è?Â&ÕøÎ]@—»s5@|s³Öܛ?ђ'ýîØ»?ì›Âhż¿àKH¾4Ù|¿ä'É oâ¿ç~þþx@ƒ¿êKý>¯"+OTHERsnr3FGL J1849.4-00573C 391?Ӎ1-–Þv?Ò¥';+z,?æ9gi4Å?Ò¥';+z,?³6§úãéý?³û÷!H?í™+£'À?³û÷!H?Þç—À¢Ñ?¶õwýà?àŒ4Ÿ®˜?¶õwýà?Ȏéšì]"?«nñÄ5Ì?éÜE™Dè›?«nñÄ5Ì?ǶBó«Å?Í'ã`"qŒ?êzoC?Í'ã`"qŒ?}6vÜm»-?‰="ÌèäK?ïœta?‰="ÌèäK?áÚFÄöG?·ñ2|ÿÚì?ÜKsÐvq?·ñ2|ÿÚì?,Ý2êpÉ?t¹×9PÆN?ï»L‹;µ?t¹×9PÆNMIXED4FGL J1850.3-0031?ã»®¿rä{_ßÉÀ8Ú¬è*÷À:A
±3ê@¤WZn@g8¥Ì®?ÈÔÌ`it?ßÅi`ì©â@'ã'÷Ó@'Ź2;<¿çHGä¿áx{Â=ä¿Ûí$S†¿é_þ"/T׿ü¾, ¿ïõEâb`GOTHERspp3FGL J1850.5-0024SNR G032.4+00.1?¼Z–'¢?ÆòêQÜ°^?ìt­/½K¿?ÆòêQÜ°^?½ÀêìG'?½¶í¹À-?ìPâ¢w?½¶í¹À-?Óòý?³t)ô¸Qª?戡¾p?³t)ô¸Qª?ՎKOè(Q?²ŸÍ®¿³™?å8ÚXëØ?²ŸÍ®¿³™?ºÄ÷NI?¯©"œ¹¿?ïì1}7?¯©"œ¹¿?€ø¸kŸhï?‹ãÝh¦Î?ï¼Ê-?‹ãÝh¦Î?²~…ãä~`?¡2=çW—µ?í°/Cu±Ä?¡2=çW—µ?Õá¨?¸K!š¼%?ï{T±/?¸K!š¼%PSR4FGL J1851.8-0007c?¼ÿÝRMw$¿Ã·—†nïwÀ8yN»NöÀ9ß:~_@UE®
@¥¦½n‹?Ð?'}rq?ƛi÷?'@hýAߞa?ø´ý먰
?ìûi,êCÖ¿çÈâ\¿ãÑ.~§¿ë5*Ø>¿éSÕj*@¿ïÍ;]ÎOTHERsppSNR G032.8-00.1?㟸&DÝ?Ô\vëf7d?ØÀ³wøE?Ô\vëf7d?ÔN b(Ǩ?ËA϶¿£?åØïÎëœ,?ËA϶¿£?Þ
'S˜ó?·Àœ›_J?àõy6Ö3†?·Àœ›_J?ß$\ó˜`?¶%wô@.?àmц3Ð?¶%wô@.?Õ"þ:`­?ÒÿÇtâï¾?åî€âϪ?ÒÿÇtâï¾?¡*ÓJ‰?±^ߨTo?îíRÎP|ç?±^ߨTo?Ùó+C?·1Ç{¿?ãp¹j^1?·1Ç{¿?£qð×eB?"s@§U"?îÈàÿH?"s@§U"<MIXED4FGL J1852.4+0037e¿âz+ÙçVU?²¾vrÍýÏÀ7*'U¯^þÀ9n@V1dý@Ë£Œ·ˆî@XçW'Ž
?³uÃ?t#?Ƕ›Ø'@¹DŽO¹@&;Á!Gù?ïƒ9L¿ÚFÿøš¿á>f7l}Ø¿éâŽÕñ9¿ç֔–ûY¨¿ì‡{‰äðOTHERspp2FGL J1852.7+0047cKes 79?ÒÄV#Ö§u?Ñr¨ËÞÓ?æÔî¬F?Ñr¨ËÞÓ?Äò•f╿?Â-ïZ8?êÃZ¦GZ?Â-ïZ8?àA=Ê»Ð{?¶²Õ£t´"?ß}"jˆ_
?¶²Õ£t´"?Öçu¬Ìɔ?°z$"Ý?äŒE)™›6?°z$"Ý?Âë}9ða?Co?ëE ±ƒù¨?Co?ŒsÜ×Ã6?¡ŽK,°)?ïŽ0Œå¬?¡ŽK,°)?ݨ2=ٓ?¶«I¦Çgy?á+æá~"7?¶«I¦Çgy?™÷W²:ò'?†'«PÁ²"?ï0EB²à›?†'«PÁ²"MIXED4FGL J1855.1-2243?î¦i¤g¦À%цÛPôÀ:f	{¸À<C{cM­2@p¾†¸ìE@Èêí+?ÅGmgaŽ?ÙÆüÿ¦@ ü ÏîÀ?èÍ®z§?ïÑGP ©Ä¿Ü´'drñ9¿ÜÊ1ç٘¿àÿà?Æ>"¿ìAÿ~Ñ¿ïÝv¾"eOTHERglc3FGL J1855.1-2243NGC 6717?lj¸£ÓŒã?Åà׎ÐE†?ê'×Ç?Åà׎ÐE†?Ç6×&0Û?Åû¨RL²?ê2J6sÉ??Åû¨RL²?áÜF'×$â?·Õ¢ ?ÜGrÜQ¶<?·Õ¢ ?Å
ò<Œ½?¥é®Ùí}º?ê½CpÜÑ?¥é®Ùí}º?¥"`&¥>?±nŸô;L?ý^²_?±nŸô;L?¢Ã#jc,<?²îX'o,(?îÓÍɐÆü?²îX'o,(?¸þ;"ü$?ªèr04‰?ìà8òœ?ªèr04‰?…ôÝn!õ?toÁ;29?ï¨,ŠU6œ?toÁ;29MIXED4FGL J1855.9+0121e¿ïÚg·k³û¿ØÕ[½•øÀ5pfB
gÀ8¡%µ¿j@	-%R@ê쑎2?™=#¡ð«#?ÎÝöjÕâ@8oÏå†6@
Çf,"ÃI?ïÀ°^×ü¬¿¨šÜ æ{0¿ã^ FÇe¿å׈b9°ü¿ëS€™¿êP="OTHERSNR3FGL J1855.9+0121eW 44?È*@gƅ,?ÐÖÚz½éä?éõoæ^µ?ÐÖÚz½éä?O
3Ž0?•»"rŸ"?Ä+‡?•»"rŸ"?ÊWµµ?²ÑM<@D‹?éj>9"?²ÑM<@D‹>ϔµ¡@¢>ÖñŠö*‰?ïÿø®W>ÖñŠö*‰?œ»ìb?¯œœIËpÄ?ïGRá?¯œœIËpÄ?`ýÞÚlÑ?mQ*V&}?ïïrÆû?mQ*V&}?ÁJ¶½@è¨?µ»Q@¸¢‹?ë­RP¯ÅÖ?µ»Q@¸¢‹>¡Ì´ R)><ñyÖu^Ã?ïÿÿÿv¡><ñyÖu^ÃPSR4FGL J1856.2+0749¿íª¯ˆ9Ê@ö>e–\ÎÀ8v(]íÀ:3ùÄ|œ3@&#«UÚ@(îñºÂß?Ù¥"Ò?Ò^zښ@{ؾr–ö@á
s(?â¿âT'nâlq¿ê3âààU¿å8Yã¡$¨¿îa¡Û‡{¿ïÿCÂw‰NOTHERunk3FGL J1855.6+0753NVSS J185612+075340?¼çT‰*qÕ?Èܕy›Ä¹?ìcnÚ±Å?Èܕy›Ä¹?¿I|†õcU?¾Ìþ\"&?ìÐo!S•?¾Ìþ\"&?Üÿ­¨LîN?´Dxöæð?á€)+وÙ?´Dxöæð?ÓýFHÊ?±	ဦ*?æ\Ûðx›?±	ဦ*?ÝÎ2—?ѧCɶöT?ë¸L{óZ?ѧCɶöT?ƒ³K¬†È:?"ÐÅf_›?ï±2ÑIÅW?"ÐÅf_›?Ï-Ci%!f?µžóýg?è4¯%¶·¦?µžóýg?"œÆÀ[^Ò?s¦swÛ'?בֿåe?s¦swÛ'PSR4FGL J1857.6+0212¿àü¡ž¿ØÛaåùÀ7••žÀ9oAÿ~ÐÀ@p7ÿÛ=@7ïZ–O?¸#¾5y?Ö½"થ0@ ¼cñA \?úv8kX?ïʙ쥰¿ß4È<V¿âùÁÍjW¿éöå¿âÙ¿ïÌn"rp¶¿ïЌ­OTHERspp2FGL J1857.6+0211SNR G035.6-00.4?–$
Yæk?¶ï…MK&3?ïNß­`\?¶ï…MK&3?œ"ݺRC;?¡¦8ïw×?ïaèµ·?¡¦8ïw×?±ò­Õ7jÕ?£… ´ØÃ?íÁªEt…?£… ´ØÃ?j˜¥	°Ÿ?[Â"¿£â?ïågZØÑ?[Â"¿£â?€j«´•º?²áØöÇ_4?ï¾UQQg?²áØöÇ_4?p'ÝÖ®Ò?{º†˜ý¯?ïß±æcï
?{º†˜ý¯?9ÍÉl?
>Aäè?ï‹˺j?
>Aäè>ò§Ö‹=ìû>íl©4¿1Š?ïÿÚ°‡"+>íl©4¿1ŠPSR4FGL J1857.7+0246e¿h¸.B#49¿Âÿƒ
6À7ô'|À9¡v¯‰Æ@ ê¿É.1Â@ü,9
ä?§!\=ú×?h'"èl?È2<Tì?ý‹ÐÓŠT¿ïàsÞ-è?ïÿàU?Íu¿æ=^ä'å¿å'$óÅ¿à™[á}3¿×²í'¶'OTHERPWNHESS J1857+026?×ïyT՚Q?Óùñ>'Wð?äCU•2Ø?Óùñ>'Wð?îôe[é$?¹ð~z%ØN?®À¹«ù;Â?¹ð~z%ØN?àÔZ‹Íå7?¶à¯Æ(Y@?ÞWJèd5'?¶à¯Æ(Y@?ë´W½Åã?³	19ÛY]?Á.¡èv?³	19ÛY]?àŸæ¢k7?ÓA[G¬ðl?ÞÀ2»û)"?ÓA[G¬ðl?èQ%OÖé?ÐYynù)?λjÀ¤[¦?ÐYynù)?äè•ß¿‡"?À»o¤Ÿÿ\?Ö.Ô@€ðù?À»o¤Ÿÿ\?â7nÅõ1?Çaej°?Ûۑ"tž?Çaej°MIXED4FGL J1858.3+0209¿ÞˆSÇ@5¿áu"@òŽ}À8øéëÀ9ûïº7žÓ@!ÅÈC¦@¤ßÎ1PÛ?Ùc²ó?­çÄgB?äÏñå‹	´?û3r@9V
¿ï™L'9«?ë|vÕIs?íœ&¨«¿á1J$ç@¿æóé;˜\ƒ¿ïú 9påOTHERsppSNR G035.6-00.4?㺳™[E?ÓÆ®‰¯†?؊˜ÍõIv?ÓÆ®‰¯†?é´p‡Ô?˜iª5?É.?ýà¯Ç?˜iª5?âuøZQ
?¸ƒ*½1•?ÛKÍ]ì?¸ƒ*½1•?èØ¥ˆ1ç?·}
¿'À?̝iÝ¿8e?·}
¿'À?ÙÏ{åöáÁ?ÓedÞK?ãB
 ?ÓedÞK?âóý&ï?ԏQµæ?ÚÓ²!Ù?ԏQµæ?ã3+"(Û?ÂK­
Ðß<?ٙ㩻®J?ÂK­
Ðß<?Ø`š°¬?ÆTsŽ†Û?ãóϲ§©õ?ÆTsŽ†ÛMIXED4FGL J1900.8+0118¿ê#O»T)x¿÷ìqþJÀ9'J HÀ:HgÒw0¹@òÉÞ/ö"@f?šIÂÂ?Ñ£#=­?Üû=£z@Ͼ¹ä'¼?þïSZ'É¿¡…¡êöÙf¿«ŒÂƎš¿ä¦ˆ*¿ìÁÓ_
+¸¿ìšƒ¿<ÁQ¿ïğá§OOTHERunkNVSS J190146+011301?ÓZ"!å?ÓÈî6?æR¶so
?ÓÈî6?ÁDõIåôˆ?ÀïI¢>‡?ë®Â­†'Þ?ÀïI¢>‡?à1ØÇNU?µt£¿-?ߝØNqcV?µt£¿-?Õ¡åøÏg?³aR—ôË;?å/
ýM?³aR—ôË;?´ËÜFÜ@/?¹HÙas¼?íf"vû<ª?¹HÙas¼?†–8‹?•¤tR³O?不zTì?•¤tR³O?À®
fg?©düÀÀm?ëü8T|¦f?©düÀÀm?‡‹1>>é›?wÉñ&¦Žq?ï¡Ó;ÂÊ?wÉñ&¦ŽqMIXED4FGL J1902.8+1451¿î.ï¯ÙT£@	&A³)À:l*pìÒÀ;½—Õt;@ cȑª@Œ$ÞܙÉ?ÇÕ{]2?[Ä}Y-T?ª!Þ:ø@|šCã…?îb÷ç,Êc¿ê»ëýê|¿ÜÔ	­þ«¿à@ï´XaÁ¿à'ààUÚ¿çt¨+,ÔOTHERunk1RXS J190249.1+145133?ï栎^Ì?fÌýæGŒ¤?i_q]CÀ?fÌýæGŒ¤?𥳐=2H?–à/BGT?…p³`.?–à/BGT?ïÁåŎŒm?€Ñ,hâ?
L§…Ž?€Ñ,hâ?ï׋l–g?W¾«§±/ó?tpº-ˆn?W¾«§±/ó?ïpÐfy ?"û¢
Fùæ?ˆ£ËÕ3¬3?"û¢
Fùæ?íé‹DŸÊ¿?»ŽtŒï½?°³¥Ûݑ	?»ŽtŒï½?ï
{p'Ÿ?™ ¸¡æ|ô?ž°'òuÇ?™ ¸¡æ|ô?ï(ϊŸß7?†èñ_l>?šæ­»ç,?†èñ_l>AGN4FGL J1903.8+0531?v'Ùèemç¿ÏPŒŠgwˆÀ8P*|«LJÀ:ešŽŒ@ØéH-–;@Ù7fžšŠ?Àä8yC7ã?ËQäç ¹@ã\[J©@˜/…)?ïkV/Ž?×!¦BõH¿çÄM¢J¿ç5†_*2¿èa.ÿÿe¿ê¹'Ñ!EOTHERsppSNR G039.2-00.3?Û'©"ZâÇ?Ôåª=DÙ?âl+5Ҏœ?Ôåª=DÙ?ŁÎ÷Ÿ^?Ão%åöG"?ê½ßŒB(?Ão%åöG"?Û¬ˆ^³¿‹?¶Ç<
?â)»Ð¦ ;?¶Ç<
?אÅÚ¡?³{¨¡Æ?ä7z¯t?³{¨¡Æ?°l'?
?ÄLƞÃâ?íòo¸cx?ÄLƞÃâ?jÄt,°_?¡|×àéÍ?ïŠTî!ŽÏ?¡|×àéÍ?ÔlGÑÐÃ?¶ð|ðº"p?åóIÜŸ?¶ð|ðº"p?"kRŅìÐ?…íiêPó?ï\¥iÓК?…íiêPóPSR4FGL J1906.2+0631¿íG¬uÐx¿ÓVŠüñ}À9½1NV¥À:JNÇä/À@%ž©xß»@˦"c§o?ÔSs¯ûî?å©Ë@Ó@;ŽK‡½Ï?þ‡ýÈI¿Æ(!\F'¿ë¾aÔU¿ØÈç$'Ú³¿í!Äuæ6¿ïÿø="ßE?ïÿ /ÄêOTHERsppSNR G040.5-00.5?ÈêAÁ…4Ì?ÐPU½÷œÚ?éÅož²Í?ÐPU½÷œÚ?Ð9Ò),Ö?ÌMhËgêA?çãë~é•?ÌMhËgêA?áKÃCÐÔ?µs{-
É?Ýhyx^Wñ?µs{-
É?ÜPì¾Ò¼?¹½¥ùŠ4?á׉ –ý¢?¹½¥ùŠ4?ÓsŒX'?Ìî
MûzN?ë?£éß?Ìî
MûzN?‰6®"‡ÉÔ?ž(=Mø¸6?ï›%E'cù?ž(=Mø¸6?ÌBAì½
Á?³3ó€?èïo"нP?³3ó€?GZB?‡k°ÁîX?ï½Åi?‡k°ÁîXMIXED4FGL J1907.6+0703¿ïC
Ô²|ó¿ÖÑ#^))À8Õi´Ï€À:ÿ¼ä!}@!L/å¾@—ºÇç‹?÷ØÎbÏ1?»LemaØ?øæbÕ¸-Ù@<‰Ên£¢¿ïÿÆ¿l'ú?ïÿþR€ÖT¿ê¢ç@k€¿æ¶a@aÄì¿é0Ձ¥‡¿ß7Cõ"VOTHERsnr3C 397?Ùº±štéj?Ö-X—Š?ã"§2ŋK?Ö-X—Š?ä¸õ¦?ÒhíAöø?֎çóij?ÒhíAöø?ß6å¯Ç®U?¸Ù
Š×æ°?àd((Ö?¸Ù
Š×æ°?êÒ÷¿ÐÌ?´˜þ×ú?Ä·°!¼Ð?´˜þ×ú?¾+Ç^y?ÉçÑËdAô?ì.Zž‡1?ÉçÑËdAô?Ò6ãä7ïÓ?ÒÃ3åú_?æäŽ
ä?ÒÃ3åú_?ßÕÚ[Ågm?Àeó3ÎÑ?àÒLJ?Àeó3ÎÑ?Ⱦ¶|±ßê?Á;˜ aŽ)?éÐR`ӈ?Á;˜ aŽ)MIXED4FGL J1908.6+0915e?äñ(I²?ۆAãz8UÀ8='ùCM]À9ÿ_tڝp@ IË%,à@$Hdà?àë¤Éx"v?Ҁ3â/µz@¼`ˆÖÓ·?ýCƒÃ˜þ?ïÒ7y…¿ádƒ7W…"¿äLg¢%¯<¿æ¢_I¿é ÃÄæN?­[ƒIBŒOTHERsppSNR G042.8+00.6?Þz†­Èi€?ÔÒÖ ¤êt?༩Ë@?ÔÒÖ ¤êt?Ô¦Ç(ŒÕÖ?Ϧ¥›°u(?嬜k¹•?Ϧ¥›°u(?ÙÔ­±©…Ë?·vfIò?ã©'+=?·vfIò?ÙÀ=AÿÔ·?¶Ýqü‰ñ?ãá_¥?¶Ýqü‰ñ?ÂÑKa¨<?ÐwRÐe?ëK­'•ñ?ÐwRÐe?›ÛŸ©Õ?­îiÐ_E¹?ï!#¹TA?­îiÐ_E¹?Î-Y¦Ë?´fD6?èt©–x
>?´fD6?—¤…cŠG?Š‹ b©¡?ïGZÛÔã®?Š‹ b©¡PSR4FGL J1910.8+2856¿Ò	*\[1@!ͦÅÒÈÀ:_:Ôd¬À<H>¼(@!w×Å#`,?ú+RÿTÿ?ÅÛìdí•o?Áq¤ƒ³ÿ?û°^òԞR@©…—Ùûß?ïøøo"¿í¦÷P.½?ÏI5¾}ԗ¿Ôÿ©ƒq¿×kr¿»l¿Õ/â{ŠºÚOTHERunk3FGL J1910.8+2855NVSS J191052+285621?ïþiæ´»š?"cüÒÌd~?)a"Ï"'f?"cüÒÌd~?ïݝ{6¾>?€W=PY­?q1BmÔ³?€W=PY­?ïðX:ó,?m‰,ä5†a?_Oï="gä?m‰,ä5†a?ïïKWAZh?E'šãZA&?`´¨îÀg?E'šãZA&?ïú÷ýýò4?BÏ]ÃUå¢?D øèÎ?BÏ]ÃUå¢?ï*ÑAs	Y?¦a}¬$Ìî?š¥×Ú5ÚÇ?¦a}¬$Ìî?ïã¡õ€³?w[ÞoÛÞÏ?l^
l«}?w[ÞoÛÞÏ?ïÝ¿þ™¶?`·Z5š?q ª5¥T?`·Z5šAGN4FGL J1910.8-6001¿î‹JáЕÀ9¢È:£jÀ:UàñFÿ™À<¸6<Òï@/H—H†'?ÿÍÃ7!Õ=?Á¯þµÓ?àݰʹ@œb^™éK?÷Ø腏÷?ïôºâ"Š;?Û:`¤¬¿ÞI
DâG¿å¾å¹,ÜØ¿ð?ïŸJžê	OTHERglc3FGL J1910.7-6000NGC 6752?¶«~Kôðä?¾O"71Åu?í*6eå?¾O"71Åu?×À%h´
R?Éß2d«?äíK¥ùW?Éß2d«?Ðôûõ¯D&?±|
ž³m?煂(]í?±|
ž³m?ÚiµŸÎUÓ?ºòP6p¢?âË%0Õ?ºòP6p¢?°;ÀG†»ì?À6Q|/·?íø‡÷8cÒ?À6Q|/·?´ÈÔÑ-M¤?»Uß•K#?ífåe±ü?»Uß•K#?±pÐ.5…c?¢ŠåªFî…?íÑåú+ä?¢ŠåªFî…?#Š£Ñc²?"×ِíˆ?ïãªÅø?"×ِíˆPSR4FGL J1911.0+0905?çÔ Û¹l¿ÆŠæ¸Ü*
À6¦»¡+^SÀ9©\¥"›@ \Y(eNä@þš9҉¥?œŽ÷Õ9Õ?¾f{µ*Ó@#,Ùb…U@Y–8¼?ä²Àü§†?ì@֟^'¿àó\îî_Å¿âYöKKWí¿æ•V©Zý¿ã\νgÔûOTHERsnr3FGL J1910.9+0906W 49B?Ÿì˪í?¹c1#Áð?ïŸ9ìŠØ?¹c1#Áð?žÄÀt»?¡ÃÜó'\¯?ï	ßü_j?¡ÃÜó'\¯?à2è¤LY?³ÐÇTÔì?ߛæ.·gO?³ÐÇTÔì?x»ÝW†¿?j1
4^ô?ïΈE"7Ò?j1
4^ô?ºِï?Ø?É0K å?ì¾$Íâ?É0K å?qmÀ8óô$?~D¥ÏŒÝ?ïÝ$ªôÐ?~D¥ÏŒÝ?å'a#=·?¶Í o{?Õ±=繄"?¶Í o{?h~ċ²?
3+3.¯?ïÿl»ÙÏ.?
3+3.¯MIXED4FGL J1911.7+1014c?íèKgvJ¤?ʑb}ù€	À9"¤ÏWÁˆÀ:C_?*¸:@öÐÑê@ÖÐ& û?ÓéLçvÇ?ÛÊދ?@
¨d©ÍÄ@z|rí2?¹¨w­áz.¿ärÑCT§¿çò›Þ˜QE¿çè§ü2ì¿ïÿàè@?ïí—䱛OTHERunkNVSS J191157+100720?àbÑÁ¤ƒ?Õ»ýë?ß:]þ|¶ú?Õ»ýë?Ûí*ù†qÒ?ÑC©'Š	?â	jƒ<Ç?ÑC©'Š	?ã‰*P‹ˆµ?¶;'qH#?Øí«^èî–?¶;'qH#?èAtϊÂ;?³)ßS`p?Îú,ÁÔ÷?³)ßS`p?ÔühÉöŒA?Ðö+Çj?åË›¹ß?Ðö+Çj?–+j‹óP?¨¥±¨¶?ïN¤«p†¦?¨¥±¨¶?Ñ~U÷›¥?·|Ü="ã>?ç@Õw2.?·|Ü="ã>?²BOou?¦oŒ¬€Ž÷?í·½\R?¦oŒ¬€Ž÷8MIXED4FGL J1914.5+1107c?º¸×âÕwÁ?r;éàåЭÀ8þ~Ä+=›À:mܺ€™î@Ú¹w/Œ`@¯P]¥?Ëô²YƒÿÔ?ØN»{ì‹@D7£~ö?úi#͏•_?ï¢á ÁÁ¿ëtŸ¢G¿âñ—‡p¢¿å߂ç¦lç¿ïêX~FVü¿ïu üÏÊOTHERunkIRAS 19117+1107?±	n<o?¹Où›'•?íݞÒF<?¹Où›'•?·þ–8º?¸×ö彐?íÀ-hT8?¸×ö彐?ÚÞY€éŽ=?µ‰{H³"?âÓ?‹8á?µ‰{H³"?Â@áDž»?¤©ÿb3Ao?ë~oǎ'?¤©ÿb3Ao?¥ýzƒm¢	?²‡ÀŸµ
?î (WÉ%ß?²‡ÀŸµ
?f÷(?"‡¥'.c®?ïºdEW€£?"‡¥'.c®?½éD'+;B?¯BŽ""Y?ìB×mº˜˜?¯BŽ""Y?p:¾˜-À!?_´Žfø?ïߊ'á'x?_´Žfø%PSR4FGL J1916.3+1108¿½Y ´"Æ=¿×ã	
¦¢À8hjª˜Å^À:#ˆY@û®a§»@$,<žìÀ?Â}BJþ+?Ï©ãhőD@€aº/;@£ -²k¿æprÄBº?ïÎ<~`ƒ#¿äyh6J>è¿ê×0h}—Û¿ì/#¿!é_¿æ=\aª¿ÝOTHERspp3FGL J1915.9+1112SNR G045.7-00.4?â[§Ôxp]?Õ©oT÷~&?ÛH°WG?Õ©oT÷~&?ÂÆ17¥?ÂRUÂ^Ï?ëNs¹ò:×?ÂRUÂ^Ï?ÙoB»ïã[?¶•8¥Gæ?ãH^¢S?¶•8¥Gæ?Öä Ð¼èË?³"éÚ¹Df?䍯—¡‹š?³"éÚ¹Df?³3Dö¶‹?̝7VÙV?홗a
¿?̝7VÙV?‡øP®?š¥Þ‡›{'?ï ÂèóI?š¥Þ‡›{'?«(^äÄ?œ8'ÛžÓ"?îM~	胄?œ8'ÛžÓ"?ŽÀ×{E?'§©¦¦Î.?ï…ûœîã£?'§©¦¦Î.MIXED4FGL J1917.0+2245?ì0g>'­ï@v®b~zYÀ:Rß&k¤"À;›%d=—:@îƉ;Ók@"%kÊSv?ƇE¯Ç?Š²?‹cÔn?Í©Ä_Z@ÁÛÍEÄ?ïÇSó¿ãt;Áw.5¿ì¶À5¯å¿ØýŸ˜¿ák¬N"r¿ïÿï0l¯OTHERunk1RXS J191710.2+224852?ïïÒ©ì´/?jipq®[?`-UßÁF?jipq®[?ïͪgi"?Žz 	iC?y*ÌQeÄô?Žz 	iC?ï£]0mí*?‡Ç€íHö?‡(³îӉŠ?‡Ç€íHö?ïð²£3~æ?C¦f$WéB?^šºsÓ!?C¦f$WéB?ï_3ñbó?—´ÜH0?"ØÉ	"?—´ÜH0?îÔ©LêêD?±£®áŠë?¢µk1Q[½?±£®áŠë?îaÄìÈ? †É]V?¦ùã°cì? †É]V?ï¥äô"o—?wñæ'm'†?††ÂÔâX?wñæ'm'†AGN4FGL J1918.0+0331?Ãö
uq=§À-ÕM¤ÎÀ:Tâó¾ýÀ<jì$·@"*ÂsW‹?øé¥e¶š?Ècêá	ðš?Èî ÝÓN@B='1Æ@Ýw"áú?ïÄ:Âs­w¿ë
Шú_­¿Çè´ÊL"Ù¿Émêi?à¿Ò€XÀ`'Í¿Ü'kÏOOTHERunkNVSS J191803+033032?ïùԙc­"?DU3*øeö?H­›0šXs?DU3*øeö?ï®6B þ?"7™ºÊÃh?"|2kè$z?"7™ºÊÃh?ïÙDG‹7Š?tp¿E#Å]?s]Ü*–:?tp¿E#Å]?ïæ·öb-®?Q¸ËW¬,?iH	Ö+éè?Q¸ËW¬,?ï÷R1{"5?PŸFIl?Q[¹y?PŸFIl?íëÀí4e?¼œûxܵ£?°§¡ùrCÖ?¼œûxܵ£?ïIe=ÏI?"+™ÿ$
?–ÓX\VzÞ?"+™ÿ$
?ﯠÁx}7?uöSWZq?"ϲ¶È=?uöSWZqAGN4FGL J1918.1+1215c¿îúd×ðí¿Ð?ºà¼ôÀ8½3€`°À:HKjaž@!"å]<@¶"}æO?ÊJ¯;At"?ÝЌÀ\¾@±JÓbé@ ,|_Ìï¿àÓí½Þ€¿âzüö`D¿ä'§èM‡¿ílzFíû¿ïúÍ%¸ m?ïGnß0҆OTHERsppSNR G046.8-00.3?àޝñ(\ý?Ó©[6:,T?ÞBįF?Ó©[6:,T?ÁØÎß\؄?Á³Þ–â}?ë‰ÌH(Éß?Á³Þ–â}?ܙa+z=o?·iF
hs?á³OjBáH?·iF
hs?ÚeR¨G²?¹ÎÑ+p?âÍVó+Ü'?¹ÎÑ+p?Éù§';èu?Çõ{þºA?遖qã?Çõ{þºA?{Ä¡üá?@æ0?ïÁv¤ª¢?@æ0?¹½MÖ«&?¦–TxyÐ?ìÈ\E*›?¦–TxyÐ?ƒÎýú³b?}Åñ.µƒÞ?ï°Ç·ÓÛ#?}Åñ.µƒÞ-MIXED4FGL J1920.8+0418¿èzžk²ÍêÀ>ˆXÿu—À9¨" [TºÀ;"×I''?@wì…#ëÃ@]ô!¥l6?ÍM›ê+ØK?ѳ]û]ÙÐ@7ã#Pg!?ý·ö|b?î€m®YD??ÛobäPÌ÷¿ÛÏ|'l+¿ãÿÜđ•¿ë	FОé¿ïÿ n4'OTHERunkTXS 1918+042?솛5X¯ø?ºP—v¹?»Ë&U:€@?ºP—v¹?ã/ë7­'?ɾ'±aÑ?Ù¡ô)¥³?ɾ'±aÑ?ëZô2cÍ?©aܬÓX
?—ä/6pÍ?©aܬÓX
?ågÔèª"?ªúžÐ¼Ð¾?Õ0V/È«¼?ªúžÐ¼Ð¾?â7LØÿ=Á?ǍüàïL1?ۑfN"~?ǍüàïL1?ÅÓîAUz?Ç{y›Õç†?ê‹8"oª¢?Ç{y›Õç†?ۇ4g:Ì°?¹‡@×ò«ë?â<eÌb™¨?¹‡@×ò«ë?Ì,¢œï?±5Í£S°?èô×Xþ9?±5Í£S°MIXED4FGL J1920.9+1408?ÄRßF|L?¢åŽå‹ŠÀ7ü֋'oÚÀ9¹°xÙ/²@µgJ0@'³Ù¶À?Ãe7'>?ÏxJAÃ@§~^ª°?õÉå"nâa¿×ÏVˁ?ïœ}^Ðoï¿èÉ5~'ñ¿é&$ÂW(¿ï9Ä6%¿å‹‰ $¸œOTHERunk2MASS J19210164+141003?ΟZÊb–?ÒM~DöÌr?èX)Mgx?ÒM~DöÌr?¬'¤4Œ«s?­R€ý׶Õ?î6Õ¼àp™?­R€ý׶Õ?×n€ÝqEú?¶ºu(Ãe?äH¿'G]?¶ºu(Ãe?½°F¦¤ç?†˜áSe¯g?ï}ÊÊÙ?†˜áSe¯g?½Õ¦HÈF?Ñ ùO6Éì?ìEK>æ÷?Ñ ùO6Éì?z'o3·Ž?†1²­?ïÊÛ!""?†1²­?–EYÙï?®ÁêÏúÑ-?ë~Ún©‰"?®ÁêÏúÑ-?6`¹Ùzù?-®]ÙlÁ?ïý3è˜bë?-®]ÙlÁPSR4FGL J1923.2+1408e?Ú)hèÛî¿ÝŠâ²_¤À5âœáL¶'À9t3poÔ¤@:'-ºM@Z}Sèµ?'d—·Ë?»V%¦'¶(@'•Râûã@É¡
&I–?ïåæä¦f¿ÌŽ¢…%™B¿á'r½Œ¾¿â'¿Asè°¿æ²*ŠF¿å[1Ÿ4c4OTHERSNR3FGL J1923.2+1408eW 51C?ºÓ(—´ù-?ÈE¬ý¤†?쥚í	`Ú?ÈE¬ý¤†?ž2slI¯?¡õwÿH?ïlÙ?¡õwÿH?ãê^ÀL-M?²ýôyÉ?Ø+Bg¥g?²ýôyÉ?0­Iµ7Ó?rí¹ñÇÜ?ï»=Jä)á?rí¹ñÇÜ?Í6{"qU>?ÍÙ!¼4Æ?è²a7cª°?ÍÙ!¼4Æ?q
÷àÜÚ"?~&†I?ïÝä$)D?~&†I?éøҟI±Ð?°kU\ø?ȵ'Ù8Á?°kU\ø?súG´]ý?¡´ëø"V?ïÿL_îÁÙ?¡´ëø"VMIXED4FGL J1925.1+1707¿½øpKŽì?á†e_UPÀ9!<MŽ(LÀ:"*—ƒ>ä@ Úº¶ö@®÷ÝÏi?ó"»äG=?Æ꛿¹"à@®Ñ9C?òÕO[2¿ë"²Dx«?ïú|"eZ£¿ää­ßKÕl¿ç–Pn­\Å¿êäÞÚ4"¿æZêg‡OTHERunkMG2 J192501+1727?ÝS8/á?Ԏ…óä,ª?áVcè{ý?Ԏ…óä,ª?ÎQØÎÍ?Ë=¨;{Š?èk‰Ìz 
?Ë=¨;{Š?ãšÐXûø?¶nB5¬³?ÙÞÊ_N?¶nB5¬³?×DF€íÑ?½ÍoÊhC‹?äyÝÜ¿‰?½ÍoÊhC‹?ÂÇ"qwš?ÆN
zxÑ?ë~Î7c¢?ÆN
zxÑ?—5ùuÈ?§"ÇP7?ïGPp?§"ÇP7?ØX5<3J?º>VZˆ?]?ãÓåaæq[?º>VZˆ?]?Ž´ºÍ"?‰'`¶'?ï…/óÉÌù?‰'`¶'MIXED4FGL J1925.3+3705?ê	Uži@#™·|¯ÞÀ;CØ>ð֗À<¹šû@ Œ6%«á?ÿ1ž½c£?зObïœ?¹Ÿï^V?ðRtý¾@àDª~ï?ïÿÅbu@¿ã+ÂüirŠ¿â`GÓÔ(¿äG@'‰?È=Qӟ$¿ïþæZ<ŒxOTHERunk1RXS J192520.1+370527?ïÿ
YãSÕ?)"W»KÈ?TÁH.»@?)"W»KÈ?ïé°À;?uTn˜—A¢?fOû}Õ¼â?uTn˜—A¢?ïðŒÕÄv?b<ß"?_úæÅ*CÜ?b<ß"?ïþD6Ül?AèÎM9ö?+¼¡œ‡:?AèÎM9ö?ïÿ:ÜY³?{Á"†¸?¼h
M?{Á"†¸?ïm˜Bg¿¾?žÆJ¤)o¯?'L÷»Ÿ4?žÆJ¤)o¯?ïèê¨æú²?qB{à¬Î?gW&l?qB{à¬Î?ï÷;"KºÐ?M;K)ag?Qˆö÷×1<?M;K)agAGN4FGL J1926.7+3027?ÝRšš@¹èÄzÀ:•ùµc$À<UÛÔ§@xY W¹O@=áâß?Ô.ËÅeÐ>?ç|}T¨@LлnÖw@Ë#ˆÆ7²?ïý± žÛù¿à¬^YQ«¿é!¨üãëͿ웭p3T¿ï÷7ÿöšÑ¿ïôUªV€OTHERsppSNR G065.3+05.7?â‰vÖ(Ê?́€Î‹X?ÚíýS®m?́€Î‹X?ÐaPÒÖQ?ÇÂ'·ÌW?çõÏW–"×?ÇÂ'·ÌW?èðã²8ï,?®mþõ¹·?Ì<q7CO?®mþõ¹·?Üà$ÊÜÿí?²,šý¯´1?áíš'€	?²,šý¯´1?ÆՈþ@ã?ÆöÌSïÛ	?êJÀoÇ8?ÆöÌSïÛ	?žçke|ý?¨RõQm‰Z?ïÄ¥×?¨RõQm‰Z?ل÷7ÑÊÛ?·±7—q?ã="d"?·±7—q?¢wØ(Ë{>?Žh½öɊ?î؂}sHL?Žh½öɊMIXED4FGL J1927.5+0154?ޖù]ÆÒÀèp—AÑÀ:Ê]†ÃÔÀ<-/à˜[¬@!ÞÓč¹?÷êSá(¤d?ÓûÒß5…?Í6ðÂuZö?ý[íœP-?@d¾Ö"÷ž¿ïǐÀI‡?ïuEâb`G¿àkbŸ1‰¿»<
rIÉx¿ØmÙ8>¿Ö0Z»¸RlOTHERunkNVSS J192729+015353?ïù2ï¡þ?IÎá2Ñz&?K4BÍM`?IÎá2Ñz&?ï²òÝüB?Åkþ'†À?ƒCH»ðÛo?Åkþ'†À?ï×eɝ?mà/CO6$?tMu}ªU¢?mà/CO6$?ïëÝ(–6?N§D{§º?d"×o	òv?N§D{§º?ïñ@³£Ó?^éàž°Ã£?]ß騫?^éàž°Ã£?:&?¹GVt¹Œê?¯w"KÁ©?¹GVt¹Œê?ïVþíŽìË?"¯áF»Ø?• "Lj˜£?"¯áF»Ø?ï¶t¸±e?vŒ7¾V?'bÑѯbÁ?vŒ7¾VAGN4FGL J1928.4+1801c¿î¥±I°ðp?ÒC.=€6À8½ŽwýhÀ:dÍcˁs@Pœ¹ʪ@>¤€}há?˔VúËë?ŀ¬"]M
@[µƒ+ß?þÏðH'2¿ï˜"}?ïÿÍgý?¿êpÓ§²a¿åÇ~)¿îÝ¡0fÐ?Ý»4‰tˆhOTHERunkMG2 J192830+1759?ÜÛÊþ¸ÏŒ?ÔFßÀøâ?á'€£˜:?ÔFßÀøâ?Üø…ñ#ÌÁ?Ð[K²¨UÁ?ჽnŸ?Ð[K²¨UÁ?áêUb¡Ð?¹ Á´ž`[?ÝÄ+U:¼a?¹ Á´ž`[?å"Pg  ‰?µ³ rI?ÔÙ_1¾¾í?µ³ rI?Áy"QÂQ?Ã?û‡d&µ?ë¹!šël?Ã?û‡d&µ?±
!~ñEÕ?¾"Õè¹Î?íÞ»ÐXÑ?¾"Õè¹Î?؀%'y.?¶üæçàap?ã¿í>Ãpi?¶üæçàap?±¹?#Yàí?§¯]hJs?íÈؽÿ2?§¯]hJs8MIXED4FGL J1928.8+3126¿âòYàWT@B÷+E((À:g²Û‰þòÀ;ë×!ºdë@Ô]ú@6?<Uñ¤?ÌÖ¬	2ٜ?½FÚ@9U?õŸf²¼€N@ðHäJlá?ïÿâ£Î¦Â¿ÐP¼{Eñ|¿íåmã2ià¿Ë'yꧩ'¿æ"9Pƒ¦¿ïÿ¸8º1OTHERsppSNR G065.3+05.7?ïñ´½¤?roÊRžc?\—ÑSShû?roÊRžc?ïwJŠpdu?œ<ÆJuƶ?'®«9u?œ<ÆJuƶ?ïœ&d׍?"Ä*^œÇ?ˆöfýy¸µ?"Ä*^œÇ?ï{AA
XÁ?rƒÛ鶘?—×å"Û?rƒÛ鶘?ïºØµçÙ?…3nÕ;Tl?Iÿc)®?…3nÕ;Tl?ì$¦§u?Ã(®äž>‰?¾ÚÏ2ÇlU?Ã(®äž>‰?î^ .3? ¨fܛ†?ªý"b÷? ¨fܛ†?ëoß|‡?ªá5äŽ@'?Â@ñ'
áÀ?ªá5äŽ@'AGN4FGL J1929.8+1832¿îFVdvÞ??Ð=çâQï6À9i>‡ûÀ:x¦'@âdc¬Î@µ€šÅÄ?ù.¤"‰—Ä?Óf|`Ρä@`µ$9›,?ößz!8?îÐ^½$¹¿ëç?¿³‰°¿rÜHÚ~*¿çz
½É#˿胦³]þ¿Ôòb~OTHERunk1RXS J193012.1+183201?ᚼ‰¹?Ô]Ú,u™?ÜËÒv"ìŽ?Ô]Ú,u™?ÓëO%ƒ%?ϧæ¶MÒ?æ
Xqí>n?ϧæ¶MÒ?ã_¹ðÀá¡?·XMO0K?Ù@Œ~<¾?·XMO0K?×=~+?À­§Q¬ß¶?äa@ýv7ë?À­§Q¬ß¶?Æ	C-ô?ËþYîo?ê}º_¯4ƒ?ËþYîo?›w7¼QKï?­J#6?ï$FBu¡?­J#6?ØT㏺{D?¼ôȝ½?ãՎ8"Â^?¼ôȝ½?—䯁2P§?š¿˜7Ã'?ï@ڃÍ2+?š¿˜7Ã'MIXED4FGL J1934.3+1859¿ÔÞ÷‹Û¿Ýó‡·aÀ8̔<b†ÞÀ:lþÀdß~@s	%˜•ä@¦b…0V	?Éлļ³?Ớua«í@¦Ó0"'@ÖJ¦Ar¼¿Ô€˜›¿äð˜ÿjÙ¾¿ç/æw˜½Ò¿îvþdŠ¿×@Ъ§Þ׿ïÿôa¼2¡OTHERsppSNR G054.4-00.3?È,o­»?Ì£îX^¼?éôä>¿"'?Ì£îX^¼?¾ZxO
@?¿|| m&?ì4°ýX?¿|| m&?àzíoë±{?´Ìŏó{Ù?ß
% (?´Ìŏó{Ù?Ûü_]Cä?¾1.ÝIX?âÐQ^
õ?¾1.ÝIX?È
ÏÐ	Z?ÇFßÐ,?éýLú½©?ÇFßÐ,?€*ïЄ}®?‰7…Bî"Ñ?ï¿T@ôçÉ?‰7…Bî"Ñ?Û †(´»D?»~Æ.£¡?âo¼ë¥¢^?»~Æ.£¡?ˆŒrà4m!?3ùªñó²?ïÎ4Uòü?3ùªñó²MIXED4FGL J1937.0+3003¿Ì/:­GmÊ@nJ82vuÀ:j´©ÀXÀ;®º××ÂÊ@ÌýÔ+»Æ@ƒπÜ3?Émõ¦à©ù?¼™:Ü?òŸ
纏?õù>ëM@{?ïþœÚñÔ¿Öz€5D…¿èў"•V>¿ì‹©¡¤ý¿ÙLªÓ}Àö¿Þþ®Ç(HOTHERsppSNR G065.2+05.7?ïö/ˆÈÐ?b]ÂK-%?S îÜó߬?b]ÂK-%?íð¬O·x?·îÀõJ'Á?°zŸ.̼?·îÀõJ'Á?ïf¿ê2°¤?ŠzgÅÏ'?"(¾ÑU€?ŠzgÅÏ'?îä×ú—$8?…Ç–f+'?¡²€Y!qy?…Ç–f+'?ïÜ¡b•Ñ?uøöÈà]?q¯N¡ø‡—?uøöÈà]?Þ¢¿±õõª?ÒN³œÇ]?à® '+?ÒN³œÇ]?íÇßVç?¡wÙù'£¹?±ÁJ@
Ê?¡wÙù'£¹?äÇíIÄð
?¼Y"ísœ–?Öp%lví?¼Y"ísœ–MIXED4FGL J1946.1+2436c¿Ø8"±*.þ¿µê‡a¢v&À9ÖPfIàõÀ;1Cót×B@î«}œ¸Þ@ëø[ÆÐ4?Дr¾8Š`?ÛLÜõ)@¨>]2àþ@ìA‰ã>¿ïÿ…@ò
¤?ïü&âAþþ¿äIE=÷²T¿á‡n¾ú|3¿ïÿú Âî'?ê<—Ëc@AOTHERunkNVGRC J194625.5+243638?îW}Ðe]¨?¶¬¿èÃ
r?ªˆ"ûaó?¶¬¿èÃ
r?êv@3ÕM-?Æ9°+gž?Æ&ÿ0ªËN?Æ9°+gž?êA/T¡¡?«Ö_tdë?ÆûCö­y~?«Ö_tdë?îd-?íð?•æFßÍ?®ù½,Ý÷?•æFßÍ?äkJ°Ê°?ÐBÝÇé/¦?×)Çjžj ?ÐBÝÇé/¦?ÑÓJLKÕc?Ñ"ÆS‹î5?çZÙÚO?Ñ"ÆS‹î5?áOoìͯ?¸>ó?Y/'?Ýa!Ü&d¡?¸>ó?Y/'?ÞAHÌ!¬?Á飬?àßsۙï*?Á飬 MIXED4FGL J1947.7+2744?ãE Ä2õ?òñBè²ÜaÀ9|Ô4 ½À;)}œ
`@¨MŽ(LO@NU:Ä÷ì?Á¸Û=ÓË?ÐÂi\ƒ@Ö,wWOr@ý%­c¥í?éìjVµï;¿áÛÌ`ëÓ¿Ùp_ùºÂ¿æïÄH™Í¿èGóÐG¿ïÿÈ¢› ÛOTHERpwnPWN G63.7+1.1?èâ+žëŠ?Ål½3Ý4?ÌwQ½"QÖ?Ål½3Ý4?ጐ垈t?Ë´Ÿž?ÜæÞ4Âï?Ë´Ÿž?ì|:Iì¡î?¦ikä[ˆ?¼-°šð?¦ikä[ˆ?é4
? «
z‡%?Ëù¿Çß/Ù? «
z‡%?Èq††Èå?Ä5p$D?éãž{^MÇ?Ä5p$D?´êA¤¾zt?»'dÓÂ,?íb·Ë'l?»'dÓÂ,?Û¼ð¡=Qð?ºðî]Hãý?â!‡¯aW?ºðî]Hãý?ËEÎ9?¨Ö8&$;z?é.¼yú²?¨Ö8&$;zMIXED4FGL J1952.8+2924¿ïPç'I>
?ðórS³À9‰"ç¨ñ%À;F"ÈŸ@£@iëw1æ@Hþƒ(?ÉçE³Z?é£opÑ#t@–¼b~?ü¯$¦}ƒ¿ë!ƒÞFqԿـaÉÁ¿Û"Êý¿³à¿ëÊ55kó¿é¥ŠÔø³¿ïüÚ±'ÝãOTHERspp3FGL J1951.6+2926SNR G065.7+01.2?Ö¹¤.¦?Í;8pü~?ä÷#-謸?Í;8pü~?Àƒa5œfu?¾éՏF·þ?ëß'²˜æc?¾éՏF·þ?á«èæv0?²Ê©N³æN?ܨ/Ü3 ?²Ê©N³æN?Íñ_ڗKó?ª´i_²E¢?胨	Z-?ª´i_²E¢?ŠšâÈKY?'/£¥7?"=å?'/£¥7?ˆˆ"´h­?'òÂæÖ–?ïÝ± žÜ?'òÂæÖ–?¹íW™µl?©Ç;|þ?ìÝ¢Tÿ
ã?©Ç;|þ?‡Sšíè·u?tÛîÅK?"H]"?tÛîÅKMIXED4FGL J1953.6+1846?ïuÅòhâÀ)ùHUÚ'À:7ÁM<ɵÀ;Ë«¢°™@OÔS©Ë@ú37dñ?ÈÈZLQ½?Ҹ϶¤l@	ç™ÅXd?ýbG‹ÿ"?ïÿþÞ÷¿àiÒ+±^²¿ç©.ݎ$¿æ.52ôD¿ïÿõƒ¥;Ž¿å¡»§
›OTHERglcNGC 6838?ìžX'8©?»0,¶ŸíN?»
;oö:¸?»0,¶ŸíN?àg¸Ø_c?̦+¥l­ö?ß1øŽOA9?̦+¥l­ö?쯺\ªk?¤±-Åx?º'-¯§?¤±-Åx?çQÚË	 Š?¦4NçÓa?Ñ\Jiì¾ì?¦4NçÓa?ä[nM˜?ËIQFˆi?×I#dÞüÐ?ËIQFˆi?°}'Dè?¹ø÷xj?íïÐOŽ2³?¹ø÷xj?àÐEaÅ?¹©É½xÆæ?ßØ_Ëu<v?¹©É½xÆæ?À"™ñ5ëR?¡ðÄ(‰"?ë÷Yƒ²…,?¡ðÄ(‰"MIXED4FGL J1955.1+3321?î ̲±Õ@WŸß-øaÀ9ë!Ð4`ZÀ;U]"̃@6¬'=@o ×{|x?ȉº¾ØBw?ÔE,¥$'1@
yyh¡ª@	S§t£•ò¿æ±Q±£{›¿æxlâÿi¿â!?èÅQ¿å§ŸVqý¿è°ù'7}E¿ïÿýFKêOTHERsppSNR G069.0+02.7?ï£5ÛÈØ?‰l'£«ì-?‡:ò‰
Ê?‰l'£«ì-?ï-Š5è3?¡¯µRÇH
?šN¹:b–<?¡¯µRÇH
?í÷O3o?ŸKµ,"÷?°G#"<Š
?ŸKµ,"÷?ï|‰6?u·4.
Í_?}Žät¿?u·4.
Í_?í=˜ÄÝj)?´B!<l–!?¶9ÚÌ|¶?´B!<l–!?ê2'¸ùӍ?ƟÁéfWð?Ç5õ±Ê?ƟÁéfWð?ê_Å0 Ý?°)%OÉ*§?ƀëã=|?°)%OÉ*§?êŠ
ô‹é¿?±ëˬƄû?Å×Ô-ÐY?±ëˬƄûAGN4FGL J1958.5+3512¿ã֬͆@J蹒]eÀ9ÀmzVÞ3À;"ëü<üá@ p8Zdz~@9{Kй?¼vY£Š^?smóÔ#?¿¹¶š†T@2õ«hN?ï<ÌQ#ß¿Ýüê6jY¿ãí÷¿¿ž¿Ú¿
|?k¦¿å"}¾Ùû¿Öh,#Ê_ŠOTHERhmbCyg X-1?ïøc®ÑP?EÃÚ?ç=?NqDkƒ»?EÃÚ?ç=?ïޏö`L¤?˜ÐÒÞO?p¸³¬áé?˜ÐÒÞO?ïëLßז?eyAŒ¿•?d³ ŽÙ?eyAŒ¿•?ïÖhüæ?[ä¾uæö?tˁw©¤¾?[ä¾uæö?ïà¥FËìR?gMeimô?oZ¹/ô%ã?gMeimô?ï»8Ыÿ?®Îj$Ä­?Ÿ¨˜ìɸ?®Îj$Ä­?ï´ð§iÞ7?†NXM€È?'ÃÖ(ø?†NXM€È?ïgÐG;äï?}Qá'Xl#?"÷òþ$?}Qá'Xl#AGN4FGL J2002.3+3246?êr§ú|Õ¶?ñL] l‡À9u_€™"À:Ò;ߪ#@
+YuO@A\Á¡ö_?Â(ü8V2¿…®Ô5Ä)ˆ?Ãjt "?ði!#¼Ñ?é9Ÿ=Èb…¿ÞD­à#¿èær@U¿ê‹¼[f¿áª‰ O«º¿ß<À»ŸnOTHERsppSNR G069.7+01.0?ï'Ï­t9Z?¦Ì¸»(ý©?L¢ñ©r?¦Ì¸»(ý©?î@5‰=š¯?´C«yHžÞ?«ü§jn‡?´C«yHžÞ?í8d*Ä?¦efh-Â?¶?Ÿë&Ûà?¦efh-Â?îQMê2?'5c¯¿Û)?®V*æÕÙÞ?'5c¯¿Û)?힣×é"?µÉnyìfV?³
áBÙ!"?µÉnyìfV?âaõÀƒ_¾?Ó
•O$7?Û<~ù@"?Ó
•O$7?쎂í/ý?«X}[Õ¦¬?»‹è–â?«X}[Õ¦¬?àå•1;G?¼mÏïʆ?Þ4՝‰pà?¼mÏïʆAGN4FGL J2004.1+2517?眾RÇ´EÀ	ÓAü#ÒmÀ:}–FþÂÀ;0ñ9" @–—G"ÎÜ@ °«.?Ô5Ä<ÛR¢?à¯/˜sÿ¬@	)5ƒo‹©?ÿê5mË	©?ïÈ8éU™?îM]®±Ú¿á‡ÜmSÀq¿è¿ø¨ó©°¿ïÿáa¯G?îRý"ªúÀOTHERunkB2 2002+25?î
vOˆ?±{¾k6å?®?(š4?±{¾k6å?ãN:—øÒ?Ïݜf0>??ÙÕcŠÐ\?Ïݜf0>??ë!$¸úˆ?§aiÙ5Üs?Ã{m½à?§aiÙ5Üs?è9ªk×r ?°¢¯ñ4?ÏVP¢7€?°¢¯ñ4?á5•{QÚé?Ìø[¦™Ý6?ݔÕ	\J.?Ìø[¦™Ý6?¶Õ€I˜Mµ?Áx«ãH9U?í%Oö•üŠ?Áx«ãH9U?ܔRD<è5?¿]³Ç9²K?áµÖÝá‹å?¿]³Ç9²K?ÅìHh#«?²NY»ng?꾄íå÷?²NY»ngMIXED4FGL J2004.3+3339?ƒŒE¤¹ƒ?ó#5#Î;bÀ82(1wqQÀ:'µÜÆ?@¨=ý;ª{@v½+o"?¬ Jžðת?{Èù-©@"ßGù"Õ@&†pG?í%^>#Ò¿ÔM€flÆ¿Þ®<Sme^¿ä?'Q¦»Á¿ê;Á!Gù¿ä«¢æIu•OTHERunk3FGL J2004.4+3338B2 2002+33?á·ºnàƒ?ÐOÏŽ=?ܐ‹#Æ>ú?ÐOÏŽ=?ÑQÜ¥¡©w?ÈúõeX…Ž?çW­/+D?ÈúõeX…Ž?ãî÷ø}2c?µ"ŸÝ÷¼?Ø"›9?µ"ŸÝ÷¼?Ü~؇.÷©?«¸ÔÍk;	?áÀ"¼h"+?«¸ÔÍk;	?´.Mçô®?³oƒ@rÔ?íz.5Bú?³oƒ@rÔ?Ÿ$0ìß?©r&&/?ïÞxh=ù?©r&&/?Ü?ªS¿ß?·¬+°Á"?áÿà*Ö ?·¬+°Á"?¤œÓ×JW§?ŒÓ¡DŒ5©?î¶2Â}œ?ŒÓ¡DŒ5©MIXED4FGL J2013.5+3613?š¢Iå}ýð?ðDq´xB1À9D5®7¶PÀ:ØÇNފd@È´p_Ž†@êC5öI?Ą‰bÙ?×Ò( °y°@zÒÁÙSÄ?øÅPt6³›¿çF3k¿Ø·Œž´`š¿á3€?ÖY¾¿çòøp¶L¿ì¯ú..ç¿ÚgzÍüwµOTHERspp3FGL J2014.4+3606SNR G073.9+00.9?çóHƒô¹?ɚӚ59·?ÑînøŽ?ɚӚ59·?ÛÈ!嶆B?Íu›MLÃ?âï
$¼ß?Íu›MLÃ?äOô·¢n)?´2/"Ã?×`»#­?´2/"Ã?åÞΚ,f?©äWu5Jà?ÔBb˧2ß?©äWu5Jà?½,u²gNv?¼wx±þ¦?ìZqI³1?¼wx±þ¦?¤ò,óG¾?°ǹ¬Mj?î°Ý0ÙLô?°ǹ¬Mj?ÌÆmFü¶?¶'F<þ¢®?èÎdœ.@Ò?¶'F<þ¢®?¸Ópmwèõ?¡ýøŸÖ¢ù?ìå'ò'ǒ?¡ýøŸÖ¢ùMIXED4FGL J2016.2+3712?í+Yy–?ñÝݖH¬AÀ9+RFòÀ:Syú—á@"5g+Þ*B@—|ˆç›?äßzÿ¥' ¿©ƒ—àÃ
?ô« b
·?ýRAüNŋ¿ÝGµ¡7?ï-.Â
Q¿ë€#¦Î5ƒ¿ãÛù%k¼¿ãKêN½Ó5¿ÜsZÀ•ÝOTHERsnrVER J2016+372?æ([†c†ã?ÓØ(ýò	?Ó¯Hó8ò:?ÓØ(ýò	?ìe¿A@^Œ?àºH{*?¼Òõýž?àºH{*?åñqÇÃ?·B$)	v'?Õéüpy?·B$)	v'?î-zÃPÞP?Ÿ;S`™+?­(SÊòÿ?Ÿ;S`™+?ܲ=:¯9¥?Óè*˜§M¯?á¦áb¨c-?Óè*˜§M¯?⠛è˜3?Õkï^¿un?Ú¾È.ÏÚ?Õkï^¿un?氕oρï?ºÝ@Õÿë?ÒžÕ `ü"?ºÝ@Õÿë?à˺± ?Ç ÔBÚ<™?ßühŠœÀ?Ç ÔBÚ<™MIXED4FGL J2016.3+4953¿ç.mÈý­@ ;EkD¹À:²€	¥›0À<`
šó5í@!èÀA¤?ø^h5sT?Îë``½Û?ÊO'åJr?üôÙáˆE´@XÛ¾­$f?ïðKAœØh?ïÿQ"W6?δ°¨©Ø¿Þ'Í»à¿È%6Æ:·a¿áБb"sOTHERunkNVSS J201619+495324?ïøË?W,-ª8t?Oçü|'R}?W,-ª8t?ïß[Q¬½Z?wrs蕍>?pRW$s?wrs蕍>?ïѳ§jp??|-v‡{ñ?w&,Ih'?|-v‡{ñ?ïº1ÌßJ?jƒí'話?xsŽ×ñ†?jƒí'話?ïó)(©}¤?^¶®)õi?Y­®µCÈô?^¶®)õi?ï.üJúáC?¥@bÆ]m?š v¥ËA?¥@bÆ]m?ï†$®yêA?_I©¦³Ý?ŽvÔkÔCÌ?_I©¦³Ý?ïf•I…?ˆV¤›cì?"-VËéþ?ˆV¤›cìAGN4FGL J2021.0+4031e¿î"‡!®Ó@'âûã:ÍÀ6ûî'):ŒÀ9ºG²F8É@!ë$ ?ýþ«×‰¿1?¦ÙÞÃð/?¯BþñüÌ@Dnœ•Í\?ö}X@?ëIÒF‰QM¿êPãèrDÁ¿åŸ£i&4G¿×Mn]UƆ¿ÜºQ,k¿ßŠoŊ¹,OTHERSNR3FGL J2021.0+4031egamma Cygni?Þxêx?"?ÓL1­ˆJ"?àÃòŠÃà7?ÓL1­ˆJ"?âXÙy>Ám?ҍÛx2õ?ÛNM
'}&?ҍÛx2õ?ãm½ý?õþ?³¥6Ea^?Ù$"€?³¥6Ea^?ÚHÃÉÿú?¾ÉùˆÂ‡?â۞ý?¾ÉùˆÂ‡?å㯬h?ÏݍpÜ?Õæ8 §Í0?ÏݍpÜ?Ç}Òby?ÎÒ>aö¦?ê »Kg~â?ÎÒ>aö¦?çödw+Ž?µáÂ~õfe?Ðý7¨ä?µáÂ~õfe?®Ç>?E†?¢4÷î'¾?îŒסè?¢4÷î'¾MIXED4FGL J2024.0+3202¿éÚ|λBÀ	,ºËCÀ9Þ Ž€`ãÀ;GµöâJ@ {¼ý@Á…pí©?ÈÚþ=Þ?¹E\U–_}?ö8N%'ö@"I­/?ïåÑ0é­?ʄ‰§‰r¿ä™þ³ú™¿è'9
gǏ¿Ì†£V‹}¿ïÿ¶ßO±COTHERunkMG2 J202410+3203?ïü¯÷\ ó?4wR¿kË?:€G.Îþ?4wR¿kË?ïÓw¯Ë?€vF¢‹ŽŸ?vD(µ?€vF¢‹ŽŸ?ï¿÷ãë'"?€ôOeHz?€ùÅ•?€ôOeHz?ïێ@A…ÿ?\Ž–î²èX?r8ß⬜¦?\Ž–î²èX?ïðìž>
?ZÖÚEœôm?^&÷Çü\?ZÖÚEœôm?ï-oß?¦¶Å¼q¼¯?šNR;í]?¦¶Å¼q¼¯?ïròw–?–pw¢?'¡·ýD?–pw¢?îûŒšFˆ?•ÒW%UÐ? G6X(K~?•ÒW%UÐAGN4FGL J2026.5+3718c?å¿\+"¿àЧLàƒcÀ9½Í!†b…À:ßöX·Q;@ÔÉEƒÃ@¥
ÙwÕú?Õvzۓd ?èfÃî×¹@
me¼{a?õ°r‹ã£~¿äsþÔV"¿èªý¤Ûìû¿Ü`wIJ¡þ¿îø‡›jT2¿¾_~8j*¿Û•Ü
Wq×OTHERunkNVSS J202726+372249?ì÷ï!nj?óÓZõ2á?¸Gx†ñß?óÓZõ2á?Ý&êTòö'?Ñ
meÍÓø?álŠÕ†"¿?Ñ
meÍÓø?è¤_̪yL?°Â0*ñïg?Ín€ÍVÐ?°Â0*ñïg?çƒw)	í?¸á×®6»|?Ðù­ì%Ç?¸á×®6»|?è†!,aT?ÎyT»Õ>ò?Íç{çNz¯?ÎyT»Õ>ò?¡ÎI5¿Y¼?­é^¶–?ø?îãl±ÈÔ?­é^¶–?ø?áV\<¹;B?¹/®?)FÜ?ÝSG†‰|?¹/®?)FÜ?³pº¯E»?µwsq½?í'è©æ݉?µwsq½,MIXED4FGL J2027.0+3343¿Ü´=-"jÀ8''
À:u¹Èä
À;…-RH¢0@#±"™ªŒ?ýgQbÉ"ô?ÅcrÁ¯Z¿®—Azž¬©?ð'¹M"‰?ú'Ÿµ<O¿îy`^dL?ïÚ­`ûH¿ì%V¿ÝÀ>Æå,¿àQù\wпá6—Á¨+ƒOTHERunk1RXS J202658.5+334253?ïûdØÐCØ?JQ0{	²?BlBTá>?JQ0{	²?îZiMKG?¸ÁVN7½Ô?ªYk*kD?¸ÁVN7½Ô?•g°¾?ˆÝ¶œ7B\?‹ÑZ°b¤^?ˆÝ¶œ7B\?ï4igˆáw?Œƒû-Ðv9?™rÓ™2?Œƒû-Ðv9?ïÊÄfn@r?€\,ÿM	Á?zÌÆ ?€\,ÿM	Á?éÒ؛üº?Я:"Ä-Ê?È´
¯?Я:"Ä-Ê?î¥B!ì?ž¤<W@¦?¥«ÝÜó;?ž¤<W@¦?趆Ü…—?Á8XaÁ?Í%䏥é£?Á8XaÁAGN4FGL J2028.6+4110e¿ß<Âݤz7?öW¾VèDÀ4–š9ŸÀ8¼ C@ZgPœ$¹@wkcü(Û?…kŒ.æ·? ¹L^ʳ@¶Ã ¢@wu2)ô?ß&2dZ™¿Ê¼˜·œcù¿áÔ<iÌ¿á¹n¡q€¿âqPÚãæſޏ¹OTHERSFR3FGL J2028.6+4110eCygnus X?Ñäx4Å«?ÓRé¹d²?ç
Ãå~+?ÓRé¹d²?ÍG°e/|?Êú –I>I?è®æ´ ü?Êú –I>I?æ'fIž?±àß¡DQ?Òû3müÃò?±àß¡DQ?Áb€¬ýhe?°TÄÐÅxò?ë§_ÔÀ¥ç?°TÄÐÅxò?à.ú® S?Ón¹52ƒ?ßõ¢
£¿Z?Ón¹52ƒ? ÁvÍÿ·7?²!Ú'\?îóè"‡­?²!Ú'\?ëSåìi±[?¬»­'±mø?°hNY:•?¬»­'±mø?‡
gðÊÅñ?'F1d"e»?ï£Ê`™˜?'F1d"e»MIXED4FGL J2032.6+4053¿Ò¯E'Ü;*?äO\"UŒúÀ8ÉRÄÈòÀ9ûtä®jâ@R
b""Š@´œU5¼?Łø4È?ÔNžÃO @óíx:¤@¨×Ðâ¿Ô(v;©Ï¿çIüm¤HI¿êêgèF¥×¿è–Ñ"qïÜ¿ëÀ©s+pÇ¿ïÇ/¿`R¦OTHERHMB2FGL J2032.1+4049Cyg X-3?ìÊv Ì0ù?ÅᖠqË?¹¬Nùžx7?ÅᖠqË?î ½Ûuå"?µ£E²'Aæ?­ô"Lí)Ë?µ£E²'Aæ?ãÉø¬¤Ž??³ˆÅ…t_?Øl¦¶ã?³ˆÅ…t_?î©Ñ:£G¡?'"ö+FÓð?¥bìZì?'"ö+FÓð?îÝF"@8w?³{U¢#÷?¢+—¹hØ?³{U¢#÷?唿äRh?ÒÞ)qút?Ôր7Ñ[0?ÒÞ)qút?æځñæ?±æ·w®•Þ?ÒKÇèü5?±æ·w®•Þ?Þ
te`5?ÁÓÉÿp–Ÿ?àÿyEÍOæ?ÁÓÉÿp–ŸMIXED4FGL J2041.5+5554?µ,Žqr@ é$Jb#âÀ:Ù­äÀ</êp'@2=²hŸ@^´UªW?Ð?ÐDÑkB?ÌÔÜeÇ6?ýeuU²Ê?÷ …[Ÿ
¿Á³k¢Š?ïäÂAÉy¿çL`RP¿ÞCиò$¿á!Äuæ6*¿ïÿîÝÃÀ	OTHERunk1RXS J204129.4+555144?ï£&í÷â?­$ÿ{¼2?‡6Dˆæ±	?­$ÿ{¼2?íMŒ)=ˆ?·joT^—‰?µ"›ÛÕ:?·joT^—‰?ï^qœÇÄ?†Q¯íek?Œ(c‹Ÿ"?†Q¯íek?î=òmµ?'†D:2$?¯~ý=±?'†D:2$?ïÌüË@?y↑ 3.?yšo…A?y↑ 3.?ఞq"_¯?ÓW`¿]x?ޞû@¢?ÓW`¿]x?í†ÛZõ
?¨eK	BèÁ?³É%+~K?¨eK	BèÁ?âŘìܝá?ºÙµƒ…?ÚtÎ&FÄ=?ºÙµƒ…AGN4FGL J2043.1+4256c?âŒ&ª	?Ô[Ý¡[YîÀ9;αð¨À:i­°hé@¤S³Ü;@O¡»§
›?×¢‰G;ÿ?í~âÿ>9!@Xt »ÌÊ?ü»ÞDno¿æ›å¿ê¿ÖO© ø³…¿ë}Žc|¿îÛ-M@$³¿ïӘc8´|¿ïø~a.ïOTHERunk2FGL J2042.0+4252cNVSS J204232+425813?ØXMá½Ó?ÓO"'vd¶?ãÓ±Y!?ÓO"'vd¶?ÈwÆë·H¬?Lj´&Bý?éâE-Õ?Lj´&Bý?ãnè©?²É6u?Øá"/æÞ­?²É6u?»~<—œ$ ?£oúœZ[?ì8m{l?£oúœZ[?ßp•$?Ô'»‡?àGô5q{î?Ô'»‡?•
>rVŠ?¡•ûAîý?ïWw®mL?¡•ûAîý?Ú$%¿]"?¸#'SWª‡?âíí Qo?¸#'SWª‡?YÀ&z­æ?N`&
ç%?ïóìÑÇU?N`&
ç%!MIXED4FGL J2045.2+5026e?æí#b
o@®…bªðÀ6ÿp·ù1À:wÖåTƒ@¢¡Åâø³@8¿E$Í?rj֍•Õ?Ì&ãÚ˜Á@*è"úô'…@dk@?á?Ä/ZöñŽx¿ÖËF…¿å‰·~±áº¿çÏ°!Etÿ¿ïGšþôgF¿ïܛ¬™PžOTHERSNR3FGL J2045.2+5026eHB 21?u4òW¯?:?'Q‹?ï'+/rx1?:?'Q‹?§%".èÃ?§Ø,mC?ÍsÎ?§Ø,mC?Ð
q/d"ö?²ª‡{gˆ?çúÇhM¶?²ª‡{gˆ?eKÌÀŽ)<?Z.ËH«þì?ïê´3V?Z.ËH«þì?w
êԜ'Y?sÁ§sW¬?ïÑê*M'ó?sÁ§sW¬?mýîߚ{?…cEŠþÀ?ïÁ$
£#?…cEŠþÀ?ã\¢(š?°vöÈZš?ë(×uÙ\?°vöÈZš>ç¿Ûöfb|>åx"L›¯?ïÿè?ïÚ>åx"L›¯PSR4FGL J2051.0+3049e?ÑÞ­1HnÑÀ ìµ»8OÓÀ77Ú¼y˜rÀ:Õçd'ÇÅ@¡ÓÏËZ@ž¸Ø#B$?˜¾"ºêø?ÉpÐãõè@-f8Éu)x@ˆÇÕGj?ïÁ´ †å¿ÕL@ËLD¿âßhæsg¿åÛ¹™ê!q¿è*'ò"È¿ê†Iàô¡þOTHERSNR3FGL J2051.0+3040eCygnus Loop?±£Ål?²7þƅe#?íÝ+‡BT
?²7þƅe#?¥|ðQÈZÞ?¨Mýx?î¨0úãzR?¨Mýx?Ý·*ÿ]Þ?´óŸ8XÐÀ?á$j€Qt?´óŸ8XÐÀ?g"¿6#
?a¨Rø¸Ê?ïèÝ@¯¿î?a¨Rø¸Ê?¤šmfü1–?¥Ápэø?î¶Y)«¹Æ?¥Ápэø?€ãÚô…µ?‹@ѧ3'x?ï¼p"pB'?‹@ѧ3'x?ß.KF>Až?µ´ã˜önw?àhÚ\àß1?µ´ã˜önw>ê/E­<³>ò®'Q'²×?ïÿåС:>ò®'Q'²×PSR4FGL J2056.4+4351c¿ï÷€ññ¹/¿ïDË ¥<À8âô2}À:¦"%¼R@ºvQëÛ@ûB+»?Â)Zl] ?ÓÆ¢[Šk@!w~¼ž?ø-c­úN»?èáºÅc¿Òô&­é²·¿åá?(‰â¿ë	ë;LÝ¿êåB_ !¿ïÿÿ>¹úOTHERunk3FGL J2058.0+43471RXS J205549.4+435216?ޝ†ÒÜ?ϗщ[D0?àðú1<–'?ϗщ[D0?Èô	Ì nN?Ħ?.éøW?éÂýŒ÷äl?Ħ?.éøW?á¢7"0?´':uíy?Ý»'»ÿ ?´':uíy?Í>Ô¾«i?¦…-¯Œ?è°JÐU9æ?¦…-¯Œ?´'†× ?¹í<??íiÄ.?¹í<??—8c½ˆš?¢U1@l?ïF<ƖÛ?¢U1@l?¾ß,Ёé?©6Åh•Æ?ì$eÿ/Ã?©6Åh•Æ?€2êZn¥?h뭈÷Ó?ï¿4WdY¶?h뭈÷Ó$MIXED4FGL J2058.7+4454¿Üfž›GU¿âçF`6¡}À9t— Ÿ³À:þºoÒö²@«œÂ˜ìK@7á2µ^ò?ÐÔbãz
b?ÉH±õ…þ‡?û}E‹$‹Ñ@P	N][%?ì¡ÚƙØ?ÝjùÞ}Ï9¿æˆž¿É.2¿ç»Sþ"Õ½¿ïø*~XËs¿ï–ü0g¦ØOTHERsppSNR G085.9-00.6?'$ˆ©?°RŸßz?R›¶ÝÕ¼?°RŸßz?ïz"^°Ô?–¤Hº¨Ò?¯t)ü}?–¤Hº¨Ò?í·>I€–W?¢|"Á0?²F
³fH?¢|"Á0?îíY܍?ˆEŽª}AŸ?¦ñ/
b75?ˆEŽª}AŸ?íÁPª´Á?±kÕõ—%´?±ó|Ðr?±kÕõ—%´?ìR §H?Á6í½]C'?½núÅ¿£€?Á6í½]C'?æŒ.hŒö?µšq—KÆ?Òç£.æè?µšq—KÆ?ç±õL?³ÄDѶـ?МgùÂ?³ÄDѶـAGN4FGL J2059.7+4837?ä2J9¬k{?ûF8Éu)xÀ:º}SèµÀ<T«@‹
‹@ÝÌÃèw£@‰à¤&?ÔÔ@ƒþ¨?îh—c^t*@¼8zšÐÑ@ªæ:²œ¿ê`ª?.>,¿ÞHšu%F¿È¢]b†²â¿Þ¼£¿ïý²6ci¿ïºýÂcOTHERunk1RXS J210008.1+484122?ì¡-zü?¹þqDƒÆ?º÷gޔ(?¹þqDƒÆ?ä·'ÈàÔ?ÍYN΢Ãm?֑°n>ÄX?ÍYN΢Ãm?ëÀº¹`¬?¨ã'×¥»?Àý™O?¨ã'×¥»?á³P‰|¸Z?¶5r×@ï?ܙ^íL?¶5r×@ï?àƒSº^L?пcyd	?ÞùX‹ÝCh?пcyd	?Çã³Zz?ʃäõ8?ê )|a?ʃäõ8?à"Çz}t ?¿²´÷ݶn?ÞÖqÀ?¿²´÷ݶn?¿¦ù‡žª?ªÃ˜ß:K?ì ÏL+?ªÃ˜ß:KMIXED4FGL J2123.9+5158?î"Â=?óhG7À9ó¼¾aÐÀ;
cûRV@¢ì1l½@¡¬Âk?ÖzРìÊ?á›Ό@@@Þ$
%'@5òzÜ?1¿í|ñýþ?•·©=ë6ß¿Üàû㐳—¿éѺ¨¿ïûR}ÔA¿ïqNŒU
yOTHERsppSNR G094.0+01.0?è#
úƒ?Çþq0Uœ?ϯsÔÉô?Çþq0Uœ?åÁß®É#?ËÔ.O?Ô}æ@¢mº?ËÔ.O?åü8JIOT?±Ë¹¢.°Æ?ԏkmaW?±Ë¹¢.°Æ?ê×µ]'Íë?¥@Ê.8¬Ø?Ä¡*‰¸ÈU?¥@Ê.8¬Ø?Ӓ‰5"'l?ɞÌ>1"÷?æ6»e=¾Ê?ɞÌ>1"÷?Âè/Ô®îk?ÇR_ÑÕRá?ëEô
ÔDe?ÇR_ÑÕRá?ÆWÕÙ)Á3?³ƒ\¸µ
0?êj
‰µ³?³ƒ\¸µ
0?Íýٗ?µf»WcÑý?耉š?~=?µf»WcÑýMIXED4FGL J2129.9+1208¿ášSâÄõ'À;Q½aõ¾^À:1'"ªLÀ<5š5 Ë½@í§°³''@?"äMòÒ?È'amÙ!?Î!µz@OjCj¸Û@ï/1?¼§»rÈ¿âè
`+8é¿åo‹^¿¿ìò_c<æ:¿æoA×:å¿ïÿ»!(ĚOTHERglcNGC 7078?ïù0¸&?CÇõu‰™?K=&/ú)?CÇõu‰™?ïßēö?uqÿ_eÓ?p{Ìùq1M?uqÿ_eÓ?ï›݅p‡?zéwj'5®?~²2HüÅ?zéwj'5®?ïà~kã?R…ñ ù$?o• KŸ?R…ñ ù$?ïôÆíKÄ?YˆüŠtù?Vr%â췌?YˆüŠtù?ïF‰ÍQ_¢?œbIpö?—.ÆM=Ö?œbIpö?îáж'L?˜ª-üpø?¡îbø‡:?˜ª-üpø?ï>}Ìœ?'(4~™,q?˜0FwfF?'(4~™,qAGN4FGL J2217.5+6346?ïæ`:ìÿ·@7hiÎÑÀ9Á²'ž«QÀ;ÆAÖd%D@!	ò«¨?ý顄I¦<?ʊ¾	w‡?Æ*"ÿ%À@I"¹`~@×èØñô$¿ï{ Ôvd?ïôx½«ò¿å/ù‰¿ÛõsŸ‰ó‰¿Ø§–ýˆ•¿ë?o¾ÁÇOTHERunk3FGL J2217.2+63461RXS J221728.9+634714?ïþ"">Ä?%JYˆd‹?/=ÛJ'³d?%JYˆd‹?ïà@+--?sküÐ?o¿Ô¡ls´?sküÐ?ïÑҕ¹/?y²*ƒÇ?wµ<¥V?y²*ƒÇ?ïÖFï0W"?\¿^_§?t܈t2ÍÍ?\¿^_§?ïúˆED"ê?ELßÝlï?EÞë;Á‹?ELßÝlï?ïć·w"?¦Wö§ŠË?œ§o¨€?¦Wö§ŠË?î¬mß?•""5?¥?ÿ½m'Ü?•""5?ï.¤ño!?‹ÏŒÍ?š=ëc‰éÙ?‹ÏŒÍAGN4FGL J2219.5+4653¿í°)Î?,À ÙXS~,VÀ;W«p_À<ˆé¦!gY@ Á"ý}™´@ÇÄ\»Â¹?ÄÀ¼ؑ|¿«å'²¶?èåRŸà¸@œw!ŸŒù?ïþ~ö€$~?»Ä‰1l‰–¿éXޛ¬C¿ßêÙþ
·y¿ìŽ°Ëæ?åÄ #!OTHERunk1RXS J221919.9+465137?ï÷ŠfSz?P@Áç辇?QòêÅe>?P@Áç辇?ïêAóüwÆ?mI'¢^ú?e¾+c±W?mI'¢^ú?ï™@¦–á?ƒälït?‰¹oÝ9É?ƒälït?ïç'gU­?Rµ;J'?héØÄ¥RŠ?Rµ;J'?ïç"ìYì?m¸?.ô?h{ûõi"?m¸?.ô?eèÖÝ?›ý¥¦¥î'?Žæ…ÊH¨?›ý¥¦¥î'?ï¢Ț¸þ?‡X‰SÝ??‡|M˓Pz?‡X‰SÝ??ïPíOF9?‡í!á90ò?•â\O8à?‡í!á90òAGN4FGL J2241.9+5729?êY©KIñ¿ñÈ÷ŠæxoÀ:!´¢3œÀ;"¾â(@Ûé	ïB@ðæ[L?Ïfr»3rH?ËÙ©T!ÀD?øö
³¸)@¤[›(¿ïd~š9Ҋ?ïþÔò5<"¿èӐÁê¿çŒ>'Γ¿îò-Lie?Óª¿^UKOTHERunkNVSS J224154+572700?磊Dh ä?ðkeé9?†ž.âh*ç?ðkeé9?ï¨rüæ‰Ñ?'¸O²ÝÈ?…ã@Í<ò?'¸O²ÝÈ?îÀS
z=š?"9%ïj?£úÏ[ËÂ\?"9%ïj?ï`ÅÞN²ô?xðâáûí?"çD=Ùt?xðâáûí?í"ñÞ÷i%?²{=¢°G?³`q	 ×?²{=¢°G?ë¶QG'³?ÅÞ¬#Æ?Á&ºáµ3 ?ÅÞ¬#Æ?æVþ½=kN?¸H[³ÎÜÄ?ÓR……)d?¸H[³ÎÜÄ?é‹'xw?´ÏâC&è?ÉÓÏbÒ%?´ÏâC&èAGN4FGL J2254.9+5802?׎Gmx²¿ö…È̍íÀ9úùXF3À;œØ_¨D@çõ±óW¦@ål†;?Æ5Ÿôým?½ó"Uâá?÷rÉìG¼W@?7àÁ÷?ïÀ"¿óuƒ?ë§xª`¼¿åÄíz¹¿äM5<ø®Ó¿ê'`eŒ¿à_ô¯iåOTHERunk7C 2252+5740?ïâæ°ké?vàZ	·?mOÏy?vàZ	·?ï"{´Î ¯?"—;øÒÛ?ŽáÚD7?"—;øÒÛ?ï}˜û 0?‡u"I¢?LàŠB.f?‡u"I¢?íRÔ8?ƒCï	·à"?§¦á(??ƒCï	·à"?íˆß'\L?´'C°j&Ì?³¹î×Kœ?´'C°j&Ì?ëð2ÖI«Î?—fÛΔÅ?À?4¦ÙPÇ?—fÛΔÅ?ìLȳ&?¯j¼|!Ø?¿eŸIºfÌ?¯j¼|!Ø?çeËÕg6V?®ð×æRÒ,?Ñ4hU1"T?®ð×æRÒ,AGN4FGL J2258.6+5847c¿×.¥4"—¿îSíPÑÀ:<§Û{¼9À;ŒV=#vþ@ E)ØÁw¯@j[{PÙ6?ÔxžaÕ]?Æ0C>Ä?ñ¾Â³nVö?ñev&wä?Ä8AåӃö?äÅhT}0¿æµAjÙh¿ÜýI׺f™¿ëqáÄ«–¿Å!]Þ,›"OTHERsfrSh 2-152?ï¹±MÚR?lªÕ®3?"¬ˆrI…?lªÕ®3?ëÌUNøì?¾wú|LF?ÀΪĐO?¾wú|LF?î™ïäèP?˜Û š×Á¤?¦a¶Y0?˜Û š×Á¤?êhd*Ä?£åµIª ?Æ_ÏöoTï?£åµIª ?íÎÒg…9)?°²So<?±‰lIJµ?°²So<?Ø=!wã«$?Òæíuõáª?ãáoD*n?Òæíuõáª?ê~líi$‡?±fŠXXé?ÆLJ[må?±fŠXXé?Мr'å‰B?³<²¹=]_?ç±Æ¾;_?³<²¹=]_0MIXED4FGL J2301.9+5855e¿çY§bœ¿ðy`>.9À8¥ÞC¯'À;jÄ$"õ@ "öøogí?ÿµè"¹7Å?¬AÒ³@´¦?«"͏@'2úÿ?@WÚœ&¿ÔEìþñb-?êÓÌ@
>¿ÞU…2à'¿átA ´@¿ã3>)[n¿ÜÔ¢¯OTHERSNR3FGL J2301.2+5853CTB 109?ï÷J±¡ož?I[€­"]?QjœmiÓï?I[€­"]?ï6jÓ2—'?¤UP÷5Îe?™2¥"…¥Ê?¤UP÷5Îe?îp‹?ðfO­KÚ?¦ÖÁ!°ÅS?ðfO­KÚ?츣Ozç}?¤
§%?º:å"(Ä?¤
§%?ï»ÏaÛõ?~!ù[y?'–÷ò£?~!ù[y?ëgµ""?ÅÈ+(?Âa+ãwwõ?ÅÈ+(?îJê$í?¢ÀšÚ_‹?«Q]¸êX(?¢ÀšÚ_‹?ä<Ç$ÛñG?¿Žé§Îæƒ?׆q¶Hr?¿Žé§ÎæƒAGN4FGL J2315.9+5955c¿Òüáøƒ		¿èOQ‹N}À9V®ÃÍIÊÀ:öÕsd{«@b‡üŽ1@jî+¸ë?ÇΊ<."x?ÇõíÂæ™ý@˜ÿàöO}?øÀÛ­:`N?ïÿÝe¡D‰¿æØO·Î8¿ä»P£‡¿é2*õw¿êìóžGÔ*¿ÞŸ‡ÜôOTHERunk1RXS J231543.9+595510?ïk²Äëà?"ãð¸?'‰½B;ú?"ãð¸?éM¼G³6½?Ä="Úùò[?ÊÉá3%
?Ä="Úùò[?íDõôŸŠÛ?¢ç§E^û?µØP\Mƒ¢?¢ç§E^û?ç$Õº‡$ø?ªßÙ4ˆJ?ѶTŠñ¶?ªßÙ4ˆJ?êlÂ4?¦>k~0æ?ÇúOø÷ß0?¦>k~0æ?ÈÄ{øý`?˳!wkhÑ?éûÎáÀ¨?˳!wkhÑ?ãÒQþ>M²?¸3r§ ?Ø[\ƒd›?¸3r§ ?¼‡7=CÀ?¢!òa9‰l?ìo]wˆ?¢!òa9‰l)MIXED4FGL J2323.4+5849?Ë>ªŽùyÀéÛÑLŽÀ7'BÁE°
À:úïY­@ۅä°ï!?ýîy	×W?šKc™å?²³	¾U÷¿@5¿jäz?ø:Șµ˜ÿ?êVð§h[?ІÁOÁs¿Ø€Jþ€ùæ¿ÞýD
öä¿ãÒRþT¯/¿Û‰°b³ÔXOTHERsnr3FGL J2323.4+5849Cas A?î›9zRµ?¶±ßtÀ?¦LhX@ú??¶±ßtÀ?Ƴ±í÷j?Â;jSÐ?êS¸Ä'&?Â;jSÐ?ê;08¬ð?¬ØՑéã8?ǯ?LA?¬ØՑéã8?ïRûÙ?¨U%,|Ž0?ë\":ëA
?¨U%,|Ž0?ë_ÿïäÔÖ?ºIÚ»3-?€@l¬§?ºIÚ»3-?˜Q܃³…&? ¾'ÃO†·?ï=q]—? ¾'ÃO†·?ì~?©–Å\?¨Qd2ÅÕ+?¼³IÕ?¨Qd2ÅÕ+?Œ'†gôÂ?€ßÅañO?ïaæ`,ø?€ßÅañOMIXED4FGL J2326.5+6122?ï£	F¤f?Ì9Ê&)_À:â¢÷ç-À;Q·ê½xœ@›, šTU@3«ÉGO?Ɍ'sZj°?¤~=šZ?à91yõd?ÿÄ¡ÿ?í¾áÝU03¿áÚñR¾¿ê7A_ƺ¿ßÍbßHOz¿êÅV¶Jª¿Ù±Þ´Ö·OTHERsppSNR G113.0+00.2?ïÙb$y¶?tâ÷^®O¡?sNíåÕi?tâ÷^®O¡?ïÂᡛÎ?…ûxÕF0?~/C ¤â?…ûxÕF0?ïUQ²
â?Žôáßî?•UÉō;³?Žôáßî?ïzšÝ*VÚ?qû6=ñ‹?¬¤SÕì»?qû6=ñ‹?îs€[Á-?©?P¤'ƒì?¨ÇúF€ã'?©?P¤'ƒì?îd"\Ìg?´0ŠÆdu?®É¶½¢Õ†?´0ŠÆdu?íAáÎ;¸?¤¾LC‰ô^?µ÷8ò×üÀ?¤¾LC‰ô^?ë¢ÿÑSf§?§U¹Ù ²Í?Átº²ee?§U¹Ù ²ÍAGN4FGL J2333.1-5527¿ëAÿÛ©ÀM)f@¦¹=À:I-(W7À<Žï¼»Ý'@í¬АÒ?ý»í·(Ú?Âz‹÷Åsè?Ô°"‡áá1@ÄÖÓõ¶?ø9‹¼â¿ÒÜ"'Z¿É§<µ¿Ü\2/ýô¿ãv=öÔ¿ë‡'aBæ¿ïý|Í°ø[OTHERbin3FGL J2333.0-55251FGL J2333.0-5535?âß ›ãÃ+?Ë=ܸò?Ú@¾È8yª?Ë=ܸò?é$ÌÏ7F?È%ðŸ\?ˇlÌÃ"æ?È%ðŸ\?à¾P!¢ß`?´pN'Ö?ރ_¼ºA@?´pN'Ö?ë0UˆÑ(?¤g¬Ð?Ã>©Ü»_ñ?¤g¬Ð?¹Ô镟'è?¶jøôØ`}?ìÅbÍL?¶jøôØ`}?ÓµÈK*B@?Ð˧pZÈ?æ%ÚjÞà?Ð˧pZÈ?¾ÀµÛLJ?©'–Øå'þ?ì'éD–v¾?©'–Øå'þ?Õބ\?ºª"W2?åu½ýÑý?ºª"W2MIXED4FGL J2357.8+6231¿ëÄ;¿ÚÝ?Ó8ªŠÀ9IëoOCÀ;0Úb·…=@qC~Yø@èÞæªÄd?Â1›X‹‡?ƾ	e"i1@QBè²Ü?÷a,Ór®H?ïÐøuÈ9¿ât1€*²±¿éÚ]C§õ}¿ç…öº «¿ïÿ4=ŸGÙ¿ïåﳁ¢OTHERsppSNR G116.9+00.2?ïLÊ9…Ãà?Ÿ8¼Ù‡J?–f¸Ôníú?Ÿ8¼Ù‡J?àöîD¨?Ì£WŽîV?ßÝÖ#v°?Ì£WŽîV?íyFtâ?¡'ñÉv?´7ÌXïÁ?¡'ñÉv?ßoé¯?±1{f|¶?àsÈp‹r(?±1{f|¶?çä£^¥Ž?ÅpMáð?Ð6¹B´ä?ÅpMáð?²&.ßtA?Àäw' ?í»=:?ŽX?Àäw' ?â'Ô+ù?¸ñѧȞy?ÚÜW©à
Ç?¸ñѧȞy?£x‹™Ø?ŠŸË¼öMÌ?îÈwNQWó?ŠŸË¼öMÌMIXED4FGL J0000.3-7355?ïåFýP´ÀE]a€M˜9À;%¦Ñ€ìÀ<ʞœ7ً@ÇÍz3£@f»üÊ?Çõ€ #v}¿®0C(É£?Û
ma'Pþ@ #¾ööA¿ïîa«ì?ìª'á›eø¿ãJ<߯R"¿àÖöâv¿ãڏÎ>¼Ô¿ïûSÞNjUNASNone?ïþ1voó?!ƒ´†"´?,è–#A§3?!ƒ´†"´?ïö>ÄÙ0?WkRŒ$s?Sé'y
PT?WkRŒ$s?ïìoîÌý?gj†ªSN$?cü;Î*ü?gj†ªSN$?ïülÌuÓ±?%ÈÒÓý?<™D`t?%ÈÒÓý?ïû(ñ!?Ah‰BÅG?C\;±m?Ah‰BÅG?ï×FIª1Ü?~=lí÷é?t\Û('aÿ?~=lí÷é?ïÔ,‡>ðx?~\ž-&z¥?ué¼A›H?~\ž-&z¥?ïîXáÿ ?U§x…ôà`?a§0zmÆ?U§x…ôà`AGN4FGL J0000.5+0743?ېÇÞ{uíÀJƒÅ?9ѳÀ:πhp+âÀ<t3⅛¶@»?ö;\?ýl½³TUÃ?Ø·G?Ëç?Þå¥vF®:@JFsBî@ÿ_Y¬Å?ï¦'ÊÖ(¿­O·½	úï¿à)HÎ¥êá¿æ™¸:lã¿ïÿãzŽ;˜?Ù­ µTUNASNone?ïü+tyÆ?Qƒïˆý	?>¤aF(¿ó?Qƒïˆý	?ïåuCè¦â?nÐâ[Ù]h?jŠ¼SÒ=ç?nÐâ[Ù]h?ïLiÏ2?‹AS÷ß?¶r×Þ¯À?‹AS÷ß?ïÍäÑj/8?`ȁ§H"•?y
—8Z€O?`ȁ§H"•?ïò—6²Å?[{>l¦·?ZÑÍÌSæ"?[{>l¦·?ïÑú'´¦?–~П?‹T³žn?–~П?î
»^ ­Ü? ÌŠý\}(?¯TJ=TH? ÌŠý\}(?ïG‡ù‰m?…¹'ސEg?—ɵˆf?…¹'ސEgAGN4FGL J0003.3+2511¿êÞ¨GîgbÀB4«ùiäÀ:¸üþÿÞÀ<|ÆÖƬ@šº²˜îú@v€$}Ê?Ð>.ϏÐ?Ԕ6ê'@\¯-•?ïÓێ¨ò?ïƹT繿à£h_Ýƒ¿à¿½‹ç)¿çk½¾<¿ïö({ILz¿ïÉÏ÷úxUNASNone?ï«ýuûÉ~?ƒÈ:ñè?…¢"}<g?ƒÈ:ñè?éF	!šb?ÅtS4ÁŽç?ÊçÛy–w"?ÅtS4ÁŽç?î+Bƒ³(a?™-ñ¯úú?­K×È=ì?™-ñ¯úú?å'ù'Ԓ?°)¿¹ 9?ÔÜÝÖVÜ?°)¿¹ 9?î¯v$Êd¾?¡È=ÖWï?¥¶ÉP"?¡È=ÖWï?ÓEKãr'?Ðç"fhƒ'?æ]ZFó7?Ðç"fhƒ'?ëVò*²ä¢?©àKöÒN?¤7U4my?©àKöÒN?Dz¥ø"?¬]ø|՝ê?ê=ÓV˜Û?¬]ø|՝êMIXED4FGL J0003.6+3059¿ßêf-4À>Å¡fµNÀ:ô™aeu¦À<ê)\ðœ@fçŒí?ýK˕•(?Ìu9èÙó§?èŸüàõ–@é™Á݅'?ý})vpö¿ê!—à¿ßAJ¸Šöi¿¨€Ua¬{¿èïÎY"ǿ隢ãÅ6Ö¿ðUNASNone3FGL J0003.4+3100?èE4•3Œ?ɆsÁ²?Îë-«3õÑ?ɆsÁ²?ãÉ&#¢"á?̋a?"ø?Øm³¸ºØ??̋a?"ø?ã¡Lƒ'D‹?³T]­ZÊ?ؽføÝvé?³T]­ZÊ?ä®ðy,ð,?°çßóÉ{?Ö¢
¦©?°çßóÉ{?ѐ¾V"™?ÌjN0S?ç7 ýTî´?ÌjN0S?ì%¬õR?Å(Únë?ëö¸"«?Å(Únë?É;\Ø7ô?³´­ÿf®ß?é±(Éø²?³´­ÿf®ß?Ĕ^Ԑ?° @CîO?êÚøhJÛà?° @CîOMIXED4FGL J0004.0+5715¿î°OÎ}Àj<´¼5À:
ö¯õ%±À;øãȑԩ@²á±
y@éÜÂä¿?Ée¶h1m?˽®·8@œC²Ý7~@Äó  ¿»ž#þ8?ï3À¶‰?¿æm4§§y¿â½˜çÂòX¿êÄò]€
׿ïý."hqUNASNone3FGL J0003.5+5721?ïˆWôý8?šx6©|"?êïqÞ?šx6©|"?ïs‡ÊlÓÆ?—ܦ¹± ?'®õë7?—ܦ¹± ?ï<%B¸>ÿ?Ç·
Ùý×?˜{W¬g¼"?Ç·
Ùý×?î‰B·	Áö?"±'|\!2?§kԒÓ| ?"±'|\!2?ëûpº/ïº?¶hªö¼žý?À=@A?¶hªö¼žý?ì´GùÏö^?À_3'…ç?º]À1€M?À_3'…ç?ç6Ut{§ì?·¼R3Ý?ѓU°(?·¼R3Ý?çè‡É–2?³3Àý¯Å_?Ð.ðlÓם?³3Àý¯Å_AGN4FGL J0004.4-4001¿åU:$q¬ôÀRvñ€
À:¤ˀœsÀ<¤@è'œ&@M®$ëò­@Ò=ÕM¤Ï?Á(òg'Ñ?´Q
u#î?ñ
	n=Ë@\nóӡӿ؍«dGRO¿â
M++ýµ¿ßdb–£¿ÞÇCuö|¿éw±b
;R¿¨ˆ¤B®ÀUNASNone?ïü°­\o?p,x¬Á?:z•`²½?p,x¬Á?ïö¡¢Ûl?W}pP­|?R¼¹Þ£Xô?W}pP­|?ïî\÷ôï?a!ÜßïˆF?a£ï1Fa?a!ÜßïˆF?ïÿ3"'ƒc?ëÞ»Ösq?›³|/'?ëÞ»Ösq?ïûWº¯œn?:õJf/]?B¡‡+Ù?:õJf/]?ïÛ&û†8?yç(;ˆ?rpl'[,+?yç(;ˆ?ïæuÀ™?toÕ=p6<?iä~÷?toÕ=p6<?ïý"¹°»I?(ú\j‡?"?3b4"ès?(ú\j‡?"AGN4FGL J0005.6+6746c?æí>¹=È@ åæyF=À9»g
USÀ;8Ś©d@«sP¯šã@Üï$©Á?ÎÿöZdÐd?Ï}Æ_@ð?Û¸"@ó…PalW¿ãŸ£i&4G?îÏ`%Æ¿ç
.Ýc¿èéRáP¿ëžÙßÚƋ¿ïÿ/?ޒGUNASNone?\æ$?‰w€0¼á?ŒÑ³Jþ?‰w€0¼á?ìq¾É gK?»Ç3
|?¼r	¶üŨ?»Ç3
|?íú'bÎßÕ?œ'y!š}œ?°+ìé‰W?œ'y!š}œ?ìÇÊ
"rW?—êXO¬£}?¹Á¯«\mG?—êXO¬£}?éã»[‹A?¿&'ƒ±?Èq'Òû»?¿&'ƒ±?ÝÇX…kÿ?Ó¦3(È?ásS½J?Ó¦3(È?à̤o?»¥Ã|½
?ßÝøf·!È?»¥Ã|½
?ÖàÔwwA?º$ª±Ê?䏕ÄD_x?º$ª±Ê8MIXED4FGL J0006.6+4618¿ÏñVf`~'À/½KÏknÀ;;·"¤%À<"g©\…<@ u™Y,í?ù,?£ƒþ?ÝQcŸâˆ÷?âi9Ÿ³äô@$ë7ò@?ù\ͶW¿ˆf_Ÿ;³Ï¿ïùš@¬ó?ímÿ"Z¿ÑÈýú1¿â%¢@Ýî¿ïÿñhUNASNone3FGL J0006.6+4618?ïø-Œé6?VÐ9ßaßJ?OIÐ[€Z*?VÐ9ßaßJ?ïè)š-=P?k¢(Çéö?gÖeëßñ?k¢(Çéö?ﲫ©;£?y®IƒŽ?ƒUÂEE–?y®IƒŽ?ïƒ!îšÛl?uŠŸE÷ü;?7"Rií?uŠŸE÷ü;?ïñÒ/•Í?^f"n¼,¶?]ô[ڍÔæ?^f"n¼,¶?ï"#>"±;?™8Û÷^²?Š÷0e²é?™8Û÷^²?ï'zÛà³V?Ž‰:=øæ?‹¡IÓ*?Ž‰:=øæ?î×o9ìh?"¶E>ç?¢‰_ˆ…?"¶E>çAGN4FGL J0008.4+6926?ï#¿ÝG°@Šü‹y£À:S\лnÖÀ;¾=‰ÎJ{@ Á<JÞö@ïþøþ"?Ê	¢Ö"0§?¸—=í§?ñi!—)|Ñ@¤5ÂÆ¿íÓbÙð!?ïþÚ0bž[¿å@£(Ž"ƒ¿åôûTŸ"…¿ÚW3£E"à¿ïÍbUNASNone?ïZÀÑt"ë?¾"—)°[0?"§åÈØ\´?¾"—)°[0?ïÜ[ÿ–^ã?vähýFöŠ?qÒóÖÃ?vähýFöŠ?ï´5—LÉ?'Üôx'Û?'ù²'E³°?'Üôx'Û?ï;ÂH?aŸ^áè?y žáx³?aŸ^áè?ïÓkÿF`{?t oiIæ˜?vJORf?t oiIæ˜?îÿŸu%Æä?¥l?^Ía? ª3õÅ?¥l?^Ía?î½DFUú³?æ4-ØK?¤+»›|;È?æ4-ØK?îi'I#"?›¼å[cÿ?©oÇÙµøÒ?›¼å[cÿAGN4FGL J0008.9+2509¿â^…›N¿EÀB\¿]xÀ:§e
EÔ À<K>I窟@îÒ09@" 5•
?ÏÎç"3*û?Èntý­ë5?ôÔb³S@â±³kÒ·?ïBO/èû׿Þf7l}ל¿êDP\8åû¿í}‡Ÿœ¿ïþž5àŒ¿ï€ú)&jUNASNone?ïø®8HW?J5$$œÂ'?MG¢·=4?J5$$œÂ'?ïáwù®#·?v±¹˜^þ`?nˆ;ÞÉi?v±¹˜^þ`?ï·fϐ?x®Åµì™?'&\@ãÁü?x®Åµì™?ï¼°2jéá?fYÒò:K?€ÓóV×+»?fYÒò:K?ïóv6Ä/?\D]ÓFðÊ?YÃJÿÂí?\D]ÓFðÊ?!"E[?—š¹ÊԉŒ?W÷¥ÍáH?—š¹ÊԉŒ?îén'G?šBƒT¾?§o¼‡w‡?šBƒT¾?î14¹ó?–áó!5´â?¯üì½<'×?–áó!5´âAGN4FGL J0009.1-5012?ßýÓÎQdÕÀPbç-¡"ûÀ:kõ²Ÿ$À<'ò®2®@ K¤ï
?@éÇ´_?ºÃˆ€l¡ê¿¿:_nÇÖ?҂ú;h@	S6Þ¹^?ïÿlýY\"¿×ö%ö4¿è>O ¿äöTðóÿêY*ÿ1£¿ïÿ"¯ý‰-UNASNone?ïýV¿¡¸n?)íÎ@B§?5J+i?¡?)íÎ@B§?ïöÐçíN?TífzÔK¸?R^/µ5B?TífzÔK¸?ïь?S?sñ¶'ý¦?w9à'ô¶U?sñ¶'ý¦?ïýì'í(?<)ߍ`?0žÁ´Å?<)ߍ`?ïüƒ:Ko.?:Ϛ† d}?;æ,å5êÓ?:Ϛ† d}?ïÛÄ È%ã?xăsâ+?r¯îN¤?xăsâ+?ïµðÝo?ƒôŒíÙHÆ?'¾ÃވTV?ƒôŒíÙHÆ?ïùjñÕ3½?=ÍÕè¤ò?JT7 Ÿ$?=ÍÕè¤òAGN4FGL J0009.2+6847?îÕðЕ·À@ðù£v'À9»œ`ô6žÀ;f?Èc@ïÓ^y@Zh+b"?É$•vjN?àÕJœ@iž»'?þ,­.vá¿Ý.Íb¿ß%"?]ä¿æ¬\꼡ܿì¥×€D¿ïÿ'`4P¿ïöU\Rç.UNASNone3FGL J0008.5+6853?èRÛ©¾?ÄgÚfµ¹?Ϻ´"½Y	?ÄgÚfµ¹?Ëû
~DdÅ?ÅÁ]LXÁ?é=`næÏ?ÅÁ]LXÁ?å÷ÃBVß?²Ý1À^­Ê?Ôy{RAý?²Ý1À^­Ê?ÎieÊ4A?©â{"-Æx?è}妍rð?©â{"-Æx?Ç»?͆—E?Ãg_RÔkÛ?ê0žZ/?Ãg_RÔkÛ?›µS¤æÖn?¥Š™>³wš?ï"Ub懽?¥Š™>³wš?ÉÌÔ܈#?¯9ÌÅäýÐ?éŒÊÈÝ÷9?¯9ÌÅäýÐ?vb™Dùœ?dê½ÎÚ%?ïÓ:ÍäØe?dê½ÎÚ%MIXED4FGL J0009.2+1745¿à#Þßý_ÀEû‰a=1ºÀ:ÊZõ1À<ulC9@õ'ßÃ@fàÄÑUÉ?Ӊ7³Ët?Öüàü.º(@±FC±/¸@uQÄ?æPËßçܞ¿æ~ُRá€PB¿×¿ëb¤À>I¿ïý¯ùWoS¿ì0>·çUNASNone?ïé6#õÊê?"Ï'YF]Ö?fÉÛߙíú?"Ï'YF]Ö?ïÑqußC?}͕pÔLH?wGE".¦n?}͕pÔLH?ïQmîšýÈ?ƒoÒ°šqÆ?•ÒB, G?ƒoÒ°šqÆ?ïiö$ã?s^÷á"Mc?'Á=4"e,?s^÷á"Mc?ï×Öö=ÖÈ?o}MŸüMY?t"ÖÅÈA?o}MŸüMY?ï%RD›ew?¡åC+ÇÛ¬?›U·cüK7?¡åC+ÇÛ¬?íœ[Hƒ°?¢–Ë¢Å??³%º˜¥z?¢–Ë¢Å??ìÆ?_;yÔ? •Ùê™F?¹Î$1c? •Ùê™FAGN4FGL J0009.7-1418¿Ü
ò®~ÀRz^³¾#À:y?Æ¿l'À<Žè´‰ßè@"êžnëp@{èäZˆ?¾ñ[¢h?¾}¹"6?ù[åô»ÿ@1är…Ùs?ïþð çkµ¿Õ÷Å^nuT¿éç`+¹Â.¿énlŒñ¿ÖÄ¿ðUNASNone3FGL J0010.5-1425?ïûž;6YP?>Yê/¯dÕ?A‡[¾ž¿?>Yê/¯dÕ?ïèÓÚ÷̚?lºsÔBê?g,$㞤?lºsÔBê?ïÔ¡À.®¿?s¡¥ÉVä?u¯ËËè›?s¡¥ÉVä?ïï~M7ì+?JE;§Šu¨?`³-#?JE;§Šu¨?ïÛŽü:V?z
•Ý©ì1?rw8ŽAlÌ?z
•Ý©ì1?ï‹á;³y.?"z.¶8?±ì–?"z.¶8?ïK	Í¢úZ?"WžX¿?–žÆMX'¶?"WžX¿?ï™.,c5Y?yÝ©gß?‰´tîá—?yÝ©gßAGN4FGL J0010.2-2431¿æl½Óa«ÀTô±î$5À;}íÎ¥!À<àINþjÕ@CÇDø'ˆ?þf ³iNx?×kWÅ®K?Å2äƒÍªm?텯¢šÜ@€­ê´iT?ïÌGkÏ[ó¿ç`.ßœ/¿åÎ=_Üßj¿¿ô/7w)¿è
˜à66¿ïÿ'¢."'UNASNone?ïùþnãì?H¯("Ñ7?HCµñú›?H¯("Ñ7?ïê*e-g?|oå¶À«?eÕé§10q?|oå¶À«?ïÓæÁ"´?p") †òq?vŸ­B-?p") †òq?ïòòÄr?CœH?ZÍås[E?CœH?ïöæÊ,'
?S˜3'Ÿžš?R2kö'ÕÅ?S˜3'Ÿžš?úˆX?')^ƒ?`?ˆØÁW
ÄM?')^ƒ?`?ï\¢'Ô˜?"j%¶¶?"k­ÀE"…?"j%¶¶?ïÓB;0O?i¬Á£¨®?v{ßdB?i¬Á£¨®AGN4FGL J0017.1-4605?ïô$|áýáÀQw_™Ã‹À:×íø–3À<©å
5r©@¼‰:Ѹ@*╶¶?Ã&LšãEµ?")ÛÔÁR?νÚÁ'ï?þ¿VGµK?ïäE#öN¿ê˜Ô½‡	Ÿ¿è–­Í-E¿ç]W>UP?¿ïþ‹ Z›¿çºñ£EêÆUNASNone?ï÷,™:Ø?P£êSæ>?Q§ý3>À3?P£êSæ>?ïâF%ö?©æ
ó?mp¹žð74?©æ
ó?ï©|ѕg?€I—sݛõ?… Ë‰x0¶?€I—sݛõ?ïè¿°jҘ?TP]C‡©)?g@OS4èb?TP]C‡©)?ïóÞ×fXÏ?\ó7j†xÙ?XBQ™Ð?\ó7j†xÙ?ï­T–§™.?•øã­u*?"ªÚcØ$k?•øã­u*?ï˜z*œz?‡Y+麑?‰áuRé†?‡Y+麑?ïTè'P$0?†)·ÿù.†?•bí´C¬?†)·ÿù.†AGN4FGL J0022.0-5921¿ÚAê‹y›LÀL°Èÿ¸²dÀ:sÕzñ7æÀ<XCëè@Ðu¡æv@…qŽ¸•?ÀŽzV³@	? !ÆyK›?áuÒ"4Ö@Wj^B«v?ïý)‹ê"n¿éb"¿H¿åVŒ¿ª¿åF^ˆ¦¿åDmþ5O˜¿ïýÒÞߞâUNASNone?ïþ-n'òË?!Ÿ´=2ò?-)Y;+?!Ÿ´=2ò?ïöJ—¨Ô?UÈc:ŽH?SõjZ{Ég?UÈc:ŽH?ïñ1æ#'^?aÉØm>?]œ3tCK?aÉØm>?ïùÉê5È?1£»?HØX£øä
?1£»?ïýZ(•us?.'÷EÇiN?5.¼: °9?.'÷EÇiN?ïڐÞù¹Ú?yIÆOáè?r·ð?yIÆOáè?ïíí£K?gS«øèœ?bô!$€?gS«øèœ?ïärëQi¡?Z|ÃWÁ?kÓ²&Q?Z|ÃWÁAGN4FGL J0023.6-4209?ÄÐÈq•»áÀR{½øôsÀ;kÿñÀ<ޟ›;ZI@â#P<@Ž­\Äüõ?ŕá"!¿ž¾¤k?Ú*Ÿü4C@ü‡ìóß?ìÁ?ûÅ¿êsÕº²¿ÌüòCÿ´+¿ã±L]üŠ€¿ïÿ Âg%?ïý<Á§TÃUNASNone?ïõ~†1¡§?ufkê=Ý?UóXx?ufkê=Ý?ïö¶À›æü?UÅ9÷šÆ?R'~¤v—?UÅ9÷šÆ?ïv—tâfM?Š[–Ýôà?'-g"ÒR?Š[–Ýôà?ïþ³ðe‹Ô?¾¡IUi?$Àön ‹j?¾¡IUi?ïû0gH[?Dü힂q?C>bÉ#(è?Dü힂q?ïÚ¬ä‹¨?y_¢x?r©·')È ?y_¢x?ï¦ýœgC?Š=yYÉz&?†@˜ØpÈT?Š=yYÉz&?ïûÆôµbè?6²%—ݦÛ?@ä,ÅL®ï?6²%—ݦÛAGN4FGL J0024.1+2402¿ÓOÍO¦ÀC4äd™ÍÀ:ÅÔɐ¥À<œ!ªt³0@Þ|§E~º@$™Ì¢Û?ÁN«^½û¿q)%ñ£"?°Ù•³%"@V½ÝñL¿ëKYš¦	?çÐP~¿ê¯ ê[S¿Á"Š‹ßœ³¿ßJâ«¿ðUNASNone?ïþ÷Âè·?ž1ìær? ŽTþ¸²F?ž1ìær?ïórµC+?]'"y".?Y•Üæjl?]'"y".?ïï÷ƒHŽ(?]·Ü©Ò_}?`|õJϚ?]·Ü©Ò_}?ïýøLòì?C¥NÞâ?0=™ 0Œ?C¥NÞâ?ïýYQLp=?6íˆìʹ?55v‹&/?6íˆìʹ?ï̏ÍÝL?FxÑ?y¸|$À?FxÑ?ïé}Ž¡?r7"ñ‹1p?f€'Pb¨?r7"ñ‹1p?ïù¾W
 9??"ê2d?I£è¼êD??"ê2dAGN4FGL J0025.4-4838?ï%Ù¾wÊgÀPú¹©çÀ:ê"ŒòÂÀ<²ÄÍúÊ6@µ·O,´?ý$ÞÚ5?Ï/®™[_?Ñ0ñd†½I?ýèú}	@@eò†ðŸ¿ã%)Ô½\¿ç濇iì-¿Ñ"…=l3¿æÒSŸd^Ï¿á&á¶hÝ9¿ïÿ«çy÷=UNASNone?ïüœß&õ?1iñÁ'ðÚ?;³C¦µ?1iñÁ'ðÚ?ïõZ"Ìä?XlæAC?UJ÷¬h¹?XlæAC?ïÌÚÞª½%?yo
{æI°?y'§1ї?yo
{æI°?ïùé'U¸?2A‰DZR?HY¼lÍõ?2A‰DZR?ïü
·ðê?;Ï¿hº>??¿"¬hçy?;Ï¿hº>?ïÖaËnuK?{Š¥ŸH0?tÏRdBt?{Š¥ŸH0?ï™#'1§?ˆnÜ##h?‰·<)ÂjJ?ˆnÜ##h?ïçèCö¤â?^,àµOê?h»á¥¿?^,àµOêAGN4FGL J0025.5-5936?Ü\«ªÆÆ+ÀL›â.]á]À:úŒð=ëÀ<bēBg"@äù~@±aCç¶]?ʾ=ö°¡?¯Ò_]ނ'?ãÁ¶¹eü@G¦(s<¿èºGúj"ɿᛃ´UÿåØ?\6a¼¿è¬x™nÑo¿ã(¥ߙX¿ç}YÇòryUNASNone?ïÿv™J¥|?ɗb9±î?,жó›z?ɗb9±î?ïöjùPÁí?UB´vѺ?S*à
†µ?UB´vѺ?ïó'CÅ/R?^ȝ÷ÿH?Xûx
-<0?^ȝ÷ÿH?ïþ&©'Q?àvÂM_Û?-•sÇ©–Å?àvÂM_Û?ïÿ…!²?ü,Q-"?¿†;âÿÏ?ü,Q-"?ïنܝ?yÔíð@iÜ?s<'Ý3á}?yÔíð@iÜ?ïï{'<‹?lÞW¤'?`"~œ?lÞW¤'?ïñ­ý8?Tc!LÜÃ?]Ü¥:•/Û?Tc!LÜÃAGN4FGL J0026.1-0732¿Ý§5t½'yÀQa 1ί%À;%sW±À< "€,á
@ fÏlå0œ?ý†»¦3ÛÐ?ÎS!¥—(Ñ?¶ cbPJ?ì7p¿°¯‹@rãºzå?íOKÝyn?Ÿj¿çdq>[°U¿¶Šùm¿¡¿ìô$)ªô5?â2ªw7oUNASNone?ïüÒuâ?4ÛgÖd6r?;÷èߔ&>?4ÛgÖd6r?ïèíX\ì?kkºž®ú§?gû'tD?kkºž®ú§?ï¹:´ºdô?|51^Ë?±RÆ
?|51^Ë?ïä"ËQ<?Vîrä?kÝ4ëntd?Vîrä?ïý'S˜ó?1.{f_Â6?3maýÕò?1.{f_Â6?ï'ÔsÊù?•Âxo"E•?‹ŠãM‹±Ì?•Âxo"E•?ïÛOŠ4l?xÂn\Ñ}'?rX:㰅ñ?xÂn\Ñ}'?)‡ú?'Iï؀?‹už<Á|?'Iï؀AGN4FGL J0030.6+0539?íýò•oyœÀLiˁs2'À:5ÆTǏÀ;å¶BFÌm@&›–Ÿ@ßR@>´q?Àª"¾"y¿¨jԊ0p
?â¶Õ^ìŸ{@÷ç,Êc?ÍïRˆ¸ö¬¿è"NÖý¨7¿ìç,­'¿éÜp
¯,¿Àò§è;é¿ï÷íA·ZuUNASNone?ïÊð³Ô$Ò?°Å%ózü?z‡¦_²ú?°Å%ózü?ïí*"…ê?jà½W›N?bÕ畵eP?jà½W›N?°A%å?"éL0ñi®?‡›"ìFê¿?"éL0ñi®?ïýqQ?Òm?%
ôàýÃæ?4uuXt¿?%
ôàýÃæ?ïÒ®wôô?†h'lT§?v¨ÄW!íÃ?†h'lT§?ï± ]\kU?‰Û é?ƒ·èŸFBä?‰Û é?ï »{ù?"EÿNë«?›èv6Û?"EÿNë«?ïÛjx*j?jàBÕýtù?rJÃîbæØ?jàBÕýtùAGN4FGL J0030.9-3618?îu…íⓀÀSõ¢œwškÀ;¹6‰)	À<꒽ÝEÁ@ ÷"	â­?ýºžavÙ?Ñ RÛÅ
;?™Émœ»	?͖z·]@΀×?ï_;#í?æë"²È?à
.A0÷Å¿â§Qa¿Ý1ð¥¿É°"‡äUNASNone?ïþ•qÁ¹H?ÅW¯ó>Š?&¨áߦ<Ä?ÅW¯ó>Š?ïô$DF?\ÃuNûTŽ?W·Õ˜pM?\ÃuNûTŽ?ïð¦gÄq?V¦Ÿv`7?_æ³gpނ?V¦Ÿv`7?ïøó¦›?:Pvoç¯?L3ùX.ò?:Pvoç¯?ïþzKm9?!'Ûð u?([J#"éß?!'Ûð u?ïÒåïCÖU?€ˆsÖ4T?v=•Ê?€ˆsÖ4T?ïîô*?k—³{p h?aÕöÀò?k—³{p h?ïð!ªìõ"?T ƒ±?_¼ªmŒØd?T ƒ±AGN4FGL J0031.0-2327?ÖÿiÜVqkÀUÃa@OÀ;ž7Åi+À=0ºö
³¸@]]àÛÍq?ùºÿèƒ?ÙÁ½|LØ?èžLa…V@
ù®º"e?þF a3÷¿ïÿãDÞVb?ïþ'AcL«?ƒ,ì6
qò¿âmSà§Ë¿í&ÕVß	æ¿ê«ßí;^UNASNone3FGL J0031.2-2320?î8&ÙCäÂ?²';ÝÓd©?¬}'o1OÔ?²';ÝÓd©?îW×Äfe©?·z¬LÂn?ª'ƒ·á×l?·z¬LÂn?ì8\	b¢?£©Ý齎å?»†=´êó?£©Ý齎å?íe)§/8?w|/ȼê?´Ö²É`¾?w|/ȼê?ê?¦úçM"?ÄR#VÐ?Çdbɵ?ÄR#VÐ?玶f®à©?ÒwT	íi¥?Ðâ"2¢>¯?ÒwT	íi¥?è¦̝kÐ?²×ùL©Q?Ígü͊PÀ?²×ùL©Q?çÙß®ÀŒ?½'À© D?ÐL@¢~çß?½'À© DAGN4FGL J0031.5-5648?ëø7ÈsÀN/Y‰ßÀ;0zW´ò»À<Ëo¤Ó‰@ A2û*?þˆåo®?ÌYO<(OT?¼\iãH;?ò@€"С@k–$ÅZ¿íYqýÌI¿Ùc"úÎg׿ۑÙüᨿà}ßÊÖS¿ÔNád‰l¿ïûs¾¾—*UNASNone?ïÿ<P	Ð?
ݗÊÒDC?uúúè±R?
ݗÊÒDC?ïöÉ×5A¼?T{dùt«?RlQ2‡Ç¡?T{dùt«?ïòƒ þ?b.;£fR?ZùÀDbî?b.;£fR?ïþ²<þŽ?Ö.Û9t?$Ü.˜}µ½?Ö.Û9t?ïÿuQÌâ'?	uÏ¡x)?UÂvJí?	uÏ¡x)?ïÚ¬•0¢?y=N•éO?r©µo‡Ó?y=N•éO?ïñ-ø"Yq?jéÅiHÉi?]¤aÒ?jéÅiHÉi?ïú‹wuŠú?> É´çÞ¦?EÒ"
ÊzÒ?> É´çÞ¦AGN4FGL J0032.3-5539?é–C	%SÞÀN á`؇ìÀ<åÏxÀ<ñ#¬­r"@$ïW'.B3?õhB>hñ[?×ñ¿Ë\ŠE?º	Þ%9Ë?ÛB¾@—õ«@#°Ó@¿êð8ÂiF–¿ïˆ!!7Þ?ëjé]Q>â¿ÄGûa@b¿ïéØÖ+?ïâ±pOô4UNASNone?ïý6d@y?SÔ쵄3'?6LÝtš_?SÔ쵄3'?ïöäPÏ?S'ë}y–Ý?R7Ý«Y?S'ë}y–Ý?ïšåT`²ü?ƒ":ȝz?‰Fªõ'°û?ƒ":ȝz?ïü(=]?;ŸÃä{}?>¾¶+f»?;ŸÃä{}?ïþ³å?%ÖlÞ¥'?!úˆ;t?%ÖlÞ¥'?ïÜé9ï¸?x9w*v¹?q‹cs‰cè?x9w*v¹?ïÎÁÏÌ92?
¦ëbž?xŸúöëT?
¦ëbž?ï÷"M¶Rs?W.VÓ?PÙd¿Vx?W.VÓAGN4FGL J0034.6+6438¿ÇNÄ:œ+?ý7ú'ص8À9›[ÖÀk•À;hb{[@<©ÏÜ@ø{,Ç?Ã؞<@£?ÄW'afÍ?@yà{Ö:4@‡å‹_š?ïöòl¬Ò¿ÍkàÊÆ¿æٚpY.o¿æ
ë­òí¿å[LVñ¿ïÿöµšUNASNone?ïÒ 3Å2?w™éqæ™?v¯æÆ×M?w™éqæ™?ï0ygþt˜?ìvHLC&?™ðÓXÖò?ìvHLC&?ïmŒ
ƒ»?‡ÊËQë˜?']®¿$œ?‡ÊËQë˜?îOŠïýB?…'
tŒä?«_'·ùÙ?…'
tŒä?홭™3u×?«ŠÉ4Kh?³2"7®+È?«ŠÉ4Kh?è^®ôÛÆ?ÊÌ5çÝ8D?·­D,é?ÊÌ5çÝ8D?éÔN'Îèö?³m:Oûùˆ?ȮŴÄ\*?³m:Oûùˆ?䨸`Ñs?±Ê¡ª2?֯ڏ>]?±Ê¡ª2AGN4FGL J0035.2-1739?ïôrp_älÀSôÏþ°t§À;–…AÂÀ<Ù¥o±"@!\Ç
Àù/?úËg<O;§?ÒßÝ5¥©?´>ïÔäžP?äYaϨÊ?ïœ,@¥·Š?ï÷òµ"¡ã¿ë¯8gOšr¿ÛöÀ›æûÍ¿Çÿfèle"¿à­ëá$
¿ÑGã¤)ÀnUNASNone?ïþBCÉ?+ãg<çƒð?+Þ¶û¾v?+ãg<çƒð?ï̺í–	Ü?Žë~ž?y¢‰UGeà?Žë~ž?ï×i1á"G?{âO*¶"?tKg/'°9?{âO*¶"?ïÒϛ¼½?`ÃÏøL>´?v˜2U"Æ?`ÃÏøL>´?ïþOYë"õ?1¹–ynþ?+
`R™;k?1¹–ynþ?îýW`l°?®|L•7"? /ªhÐý?®|L•7"?ïÞQ}è?y°¸duù?pÿWIw3?y°¸duù?ï"§<D?XÄvÃÔ÷?œ‹žÚ?XÄvÃÔ÷AGN4FGL J0037.2-2653?Ўl¸Ì ÀUµI''>À;¡éhäÅèÀ<¨,¤£¸×@"ðE¢Ìs?ì>vþdŽ?äy(_ð€†?ïäkß÷÷É?ù–wƒÅ?ýû†5ä"h?ïó°0´Ó²¿äÍp@"Õg¿ß{W#ÓCß¿ØÇáÖt@¿ïÿÆTǏ¿Í¥˜¯cÛUNASNone?ï¿Cu(Sº?¥¯Ýæ?€/"ÆÁ'x?¥¯Ýæ?ï֖ý)ƒS?ŒPf<""µ?t´e
I?ŒPf<""µ?íþÁ¬]@£?› J7ܐ9?°	ò›Ì k?› J7ܐ9?óPÞÚ?xwáé_™´?‡2§–?xwáé_™´?ï[èý¹*?˜z
 /?"'àfÿàÃ?˜z
 /?ï1R'/?¬ÛÏV"?™Õ½6VÔ"?¬ÛÏV"?î/)¤FÏP?ž8ƒ¾¶ÀŽ?­
e¹Û=?ž8ƒ¾¶ÀŽ?ïy×Û&_n?ªR÷J?Å [|>?ªR÷JAGN4FGL J0039.1+6257¿á¤¼"ÙÛ?¿4GÛ5ñ)À9Xº'Gm}À;ß|ÊUú@oeÉÞZê?þ|óÁ-\Z?¾Í³ýsß?áú|2€…Ì@ Üa•FN@åÄè4Ý¿áP"G!ý¿Ú祖'R¿ÈëJw—¿äÉ"=—*¿ï6©Àd¿í ˆ JxIUNASNone3FGL J0039.3+6256?'{¶‹–?°Ý!	K>~?ïo§4YEc?°Ý!	K>~?¸h»Ê'¡?¶DVF ²Ä?ìòÿˆO´?¶DVF ²Ä?ªÁ˔wøˆ?›³ØEb?îSãFá»Ç?›³ØEb?³¦"î3?—ß?Xѧ?í‹-'f™‰?—ß?Xѧ?–_¿€ýÏ?¾A±Tù?ïM¢-3a?¾A±Tù?Œ‹Mo'@x?•7͟ü!?ïÒÊxð¾?•7͟ü!?‹}Yµ˜"?yÇ@EëFµ?ï'
™'N?yÇ@EëFµ?eßK4Ê¸?VG¤åî(?ïê ´ø½
?VG¤åî(PSR4FGL J0039.7+4203?ÕÒ³'À4Áæ>ŽÀ;4ebZhÀ<yÏÛu<@È8ªky@ãp¥"‰g?Æ~ÈÈ[N?—Œ|ù?Ò¤_۲÷@)N^³¿Ûè®àR»¿ÊCBtï–%¿êbÙð!¿áîmØJ¯¿à?ûÞ]Bü¿ðUNASNone?ïýÎœ¨?%~
4îÄ?1a$vS>?%~
4îÄ?ïõbnEi'?W#×p
"?U;#(6rˆ?W#×p
"?ïèþ¡†"?g'ÏÄ Y?g^·¶ß&?g'ÏÄ Y?ïü¿?$Q߈F??¿¦u¬sÌ?$Q߈F?ïùTrьX?Hõ-B#?J®4©Ý=Î?Hõ-B#?ïÔ0ACõ¬?|ØÿZ–8?uçßz1õõ?|ØÿZ–8?ïÓóå6?zM¾_°Äu?v
Zc}C?zM¾_°Äu?ïè2†Ko?Yïë[hfˆ?gÍîD¨ú?Yïë[hfˆAGN4FGL J0040.2-2725?F¨'sÀUßµà÷üüÀ;BH­î»4À<|ڀ·@jõ['@‡wÞ]îÉ?Å^j™{炿ª Xz•rn?ãö«ù®r?ùÜÚ
Òüg?ïÿýaw¿êÖa +n™¿æƲ×XA
¿Ú~YÝA¿ïÿã_¶Hý¿µ	-%RUNASNone?ïî)ôùš>?b3¤Ï#~?aÖ
Á­'}?b3¤Ï#~?ï«£aÄk)?Ÿá Ÿei?…'™4	–?Ÿá Ÿei?ïó:¹~*?">#®Sµ?˜­÷¤±?">#®Sµ?ïΞ•p®Ù?c'"}?x°µM×ß²?c'"}?ïä[Vp`?mÀKÒîÒ??k¤ðà‰_h?mÀKÒîÒ??î[*º'Œ&?¶f*]Iý½?ªMTUCˆ©?¶f*]Iý½?ï!6Àô8?—µÁ²+O©?›Ù>Js?—µÁ²+O©?îïa³_z? =m¡R§k?¯Á	äÊf? =m¡R§kAGN4FGL J0040.7-7157¿éÐsa˜TÀF'³¿µÀ:ëHɝmÀ<±'¥‰'å@ ¥×Û?ý%=§*|?Ì&ÝåMø?ÕI7º@fÚå"Cï?ùš¥]G.?ä)€,
¿ïA["Ì´?é±Ç2ŠA¿áPÍ ¿æh›ÊÌA¿äÀ;#Â|èUNASNone?ïøI•Rì?EIMö0à?OŽÙ^֋·?EIMö0à?ïÆÔØ+r?…uöº!‹?|•"	ã\Ê?…uöº!‹?ï™T^á.?'òÒ÷²tI?‰ªþk·Pg?'òÒ÷²tI?îËL÷væß?'ìiV?£K0‡µ«?'ìiV?ïî÷æŶ?\Tà"éUh?aüpìa?\Tà"éUh?ï8S̎l?¦C—jû?˜õ†u´d?¦C—jû?ïQ:¬4ô?'å:+õÒ?•Ø¼,1/z?'å:+õÒ?ë÷4‰Në?°èM»šh?À#-ùÚÄT?°èM»šhAGN4FGL J0045.8-1324¿àÉ+n)¨ÀS
¥¹bŒ½À;§/F>¨²À<ò×;»—ñ@ rj Z=Ž?è×ÄýËrZ?ñ')bÏÙ?ì/"YÒÚ?úÀ?ö@Wÿ÷òjk¿î'ËâA(>?ïþCÒ½§–¿ìCʟöÕà?Æ#ˆIe$¿æÅ&p­¿ïþz#²Œ°UNASNone?ïö1?ñ.?{ø¨D6L?S€%³w?{ø¨D6L?ïèp7(=ê?tAdŽöً?gÈÈ£ÍÆ?tAdŽöً?ïbP²þx?‹ƒ™Di?"µéœÁ`@?‹ƒ™Di?ïïãŒÔå?RÀ»ø6X'?`ëTî‹?RÀ»ø6X'?ïÚä<'?u[ÂlKU²?róyY??u[ÂlKU²?ï®w&¨
v?‹-"íûI!?"b6f{'€?‹-"íûI!?ïZՁ¯Ë"?õ9~î÷?"¥Oʍ¨?õ9~î÷?ïèŸJLn1?h"'Ž;Ë?g`µ'•Ž³?h"'Ž;ËAGN4FGL J0045.9-2021?áÔ?cSrªÀTÇƧÀ;2/Ú¹šÀ<Ƨ?tŠ@ 5jE8?þõÄ}î?Èüí¦â'?¦GáýÛ9?áíÜçÍS@‡
íC峿îåNCZ?ïô¬ç#¿ânZ†^Sr¿àL0Z:ß¿Ô&2™°?οêT^/
ZUNASNone?ïþº€D?…;í¡œ?$Wÿ?…;í¡œ?ïî
ða/#?g%.¨~ø¥?aòâ)5?g%.¨~ø¥?ïðÏfb¾?c»BÙô?^a2õ˞¤?c»BÙô?ïündzÞ?*w÷aHE??d‹&žò…?*w÷aHE?ïýäù® ?&Sz
¾?0Ø0Ú¥q¬?&Sz
¾?נּ́
î?zoc¹X"?"ŸÌ˜ÝL›?zoc¹X"?ïðƒ>þo?h°}³ú`á?^ù'ViÀ¤?h°}³ú`á?ïð±XðÃ?T5›ŠåíŸ?^ó£TÉ%?T5›ŠåíŸAGN4FGL J0046.7-7048¿Ô®×˜F¢ÀG'ž@ÈG,À;œ¥R4€À<ÒÆ»:Ô@Ӑš—@¸j$aY?ÇÖÎûtU¿¨ÍÆᕦ?â³þÕ]•@¢Äþ¢1ï¿ïü]Ä?ït£`Aß¿çÄyA¿àèõW/'¾¿ïþ5Å´ª—?ïöÇ<jšUNASNone?ïõ§^J°u?_W£óEx?T±C#'6Ð?_W£óEx?ïò}N=r?`ŇËÉ<)?[c.}?`ŇËÉ<)?ï'3õ-œ¤?…®ZB??‹sÂWFñ?…®ZB??ïø˜¯±*|?>A7,ŽI?MA)¾uL?>A7,ŽI?ïçÑàÝÐÖ?m5JÄÝ/À?h.=¬	¾?m5JÄÝ/À?ï¾ðÖ
à‹?‹H'ê"É?€Cʃ¿G?‹H'ê"É?ï§êˆÛ—|?‡Ë°×ž™?†]¾ËM?‡Ë°×ž™?ïº!õ{Ë0?yg¸ ˜Úä?w'ªT%ì?yg¸ ˜ÚäAGN4FGL J0048.6-6347¿Ñ¤L`*ãÀJªÄÑ¢À:ÇK^£#†À<Çdl'"Ó@)?ý<Aÿ~Ñ?ÇÎÔcïé‡?ÚèŸ%ʔä@¦Kaþ"@.ï\ڗ¿ð?ïÿÿ)@k*¿ÙHÅ×Eî¿ä¿Ä}îB¿èÙXáÃ~ð¿ïû²]µ½½UNASNone3FGL J0048.1-6343?æ§5©µ?Él<˜{{:?Ò±"á謖?Él<˜{{:?í#DÜ0¡?½]%cւó?·&åÙzü?½]%cւó?åk?µ]ֆ?³]݇®U?Õ)€•DRô?³]݇®U?íïí½w9?"/ŸZڊ?°€'µ±¸?"/ŸZڊ?К!–uT?Æ4xÃ
VE?ç²ï4ÅsV?Æ4xÃ
VE?â ú"ŽË?Ò¾öΆ"á?Ûܾ
Öâi?Ò¾öΆ"á?ÔÖKùJ%µ?¶Gà|GO?å"ÚZí%?¶Gà|GO?ãÁ˜r
tÄ?»Ä–ûãq?Ø|Ïåx?»Ä–ûãqMIXED4FGL J0052.1+6444¿ìB´iót?ýíözE@À9y\–$À;Xfêð¤B@•ËÊï'@è‰͟[?ƪH(äj?Ñ-P›#•@Ý ×ç?öؤ^™"d¿Ô=ՃT³¶?éµ{âÏm'¿ß§›š¥³-¿ên¶—b&¿ëRæ÷ñ=Å¿ïݥ̈́'±UNASNone3FGL J0051.6+6445?îÂfWû?£Ñ"Þy›?£ÙŸ7üM?£Ñ"Þy›?âù!Òã'?ËôÒdç5Y?Ú
õ¼Z8Ü?ËôÒdç5Y?ëÅ™»
Ä?¦¨#iú`'?À띙Èñ?¦¨#iú`'?ãm̉à?°%>xÃ?ÙÕ$gÆìA?°%>xÃ?à xìƒ?ÊaÚn(°?ß¿&ùù?ÊaÚn(°?»Ø9Io,*?ՌH*?ì"øÖÒ{?ՌH*?ÜVž¶þž?¸:`Z"s?áøÔ°¤€±?¸:`Z"s?»̨Jó?¢R4Kß?ìžfjö¡?¢R4KßMIXED4FGL J0054.4-1503?浿~ýÙWÀSz îõÀ;íNäHÀ=]¹ïzw@!'|`Â8?ôÈ͙{f©?âf~x+
?êT•ƒŠcœ@
ŠBä?üù'ó¸¿ïÔwéR?ï}WÎÂ?ïéR‹¾?Ò¹,;È-+¿á‹Y/F>©¿ïøu'ST;UNASNone?ïâÉÀÓÅ?mtFlٙ¥?mê6U)º¨?mtFlٙ¥?ï5;è}FA?¬êW s"?™X'òê?¬êW s"?ïZ<p.?ˆ¯e²1"?"¸qø ":?ˆ¯e²1"?wØ1c?•Ý0±Ér?§"ƒXÐ×?•Ý0±Ér?ï»Ažt¹?'š<‰J¥k?/˜R«vK?'š<‰J¥k?íuç*qÅ?ÃTPöMàÅ?´PÆ«-gX?ÃTPöMàÅ?îݎյ"?š>ɧCõO?¢'¥ŠmÌ?š>ɧCõO?쐗bK›?²`3­'±?»{Dë}£*?²`3­'±AGN4FGL J0055.7+4507¿Ö—µqo¯À1½šA_EáÀ;ùÕm…>™À<ý3þ4Må@"¯e3?÷(ÄDhÝ?ß÷×\È­Ù?æS"ÛÈ@a.á"Úî@$m/ƒPW?ïÎT 鄓¿ïÿûÞ]Bü?ïÿ)vP¿ÍkØUÁþh¿Ì¼Õ~@"¿åÓ6þï´®UNASNone?ïùˆ—h½?DŽfrOå??K•Ý¯Ž¿Á?DŽfrOå??ïçÉ5"?kYš³Çƒ'?h6ãêEË?kYš³Çƒ'?ï£Ú—)––?}«2­V+Ý?‡	Z+K†‡?}«2­V+Ý?ï—QÖ6'ô?xSJ@)s?Š+Š|®ø?xSJ@)s?ïô*N´2?[írjpÙ&?W«Äæå¬â?[írjpÙ&?ï'[íf H?–d~eÓÇÒ?‹i˜™~?–d~eÓÇÒ?ï"í}ž¼?Y†þØ'?‹¸I|ý?Y†þØ'?îál'à2Ÿ?šôp©ð±?¡é=†HY
?šôp©ð±AGN4FGL J0057.5+6814¿áð´<ÕjÍ@{ÔÝ<†™À:aGzÕÀ;'Ö*'ò@4¥Ó
ه@ºNz·VC?΃†d9»?¥n…ž?ßiÈñuù@¯>dÐÂ?Á+¡C‡Z¿å­VŸôÒz¿ëŸH˒:¿åTê"H)d¿ëŸ¤À¿"j?µ§\лnÖUNASNone?ïç7qô?–iéÜ/ÉÐ?hÈ𞊌?–iéÜ/ÉÐ?ïåî?ýà°?pVY£l?jÀ)úÈ?pVY£l?ï}_{²ö.?†^ƺ(?T'Â=?†^ƺ(?ïä2í=/¶?QP%#Qq?kÍÀ™³?QP%#Qq?ï‡6¤)´?Žƒ<ÊRø?Ž2Vûu'å?Žƒ<ÊRø?ïÃAL?¤Djý–¿?œÜ§•˜ž–?¤Djý–¿?î
€Š\˜e?¡]ÃSk&?¯W÷X~«³?¡]ÃSk&?î±r6[å7?"'Å9'
}?¤èܜÕa'?"'Å9'
}AGN4FGL J0057.9+6326¿Ú¦Prß?ânù´
3À:{›eK´3À<-yøêb	@"óXˆØ+P?õ~€Ǒ$?̾ywæž?ÌÂy6͜€?ùۑÁ^Á@pUÚ'(c¿æòI~N9Ÿ¿êÊE3÷Å¿æÅp'Iü¿ÔSÈ
L4¿×Á'è|U¼?´°bÞÇv!UNASNone?ïúM2&²‹?A]ù\Oh?FË6bÓ4÷?A]ù\Oh?ïã8ÊC?y,'¬Ø?lÇä0oÍ+?y,'¬Ø?ïç~ü½§?dø7Pýˆ&?hU	?dø7Pýˆ&?ïö™°r4?Aùà"pþ
?RÌ N‹ö?Aùà"pþ
?ïû0FôS??xUÊ-?C?úFgÙ??xUÊ-?îÒûûø?±'Œ¸ý»l?¢ßM(r}?±'Œ¸ý»l?¼	Ž¨?ŠÐˆ‹æ?ˆ'ZÆ?ŠÐˆ‹æ?ï׺äñ¡?l´[þ¢?t"±.ƒo?l´[þ¢AGN4FGL J0058.1+6915¿àþoU½¯@–tŽGVÀ:AVZ¨WÀ;¶o×ÿ/ö@ÊæØf³é@˜±¨ó?Ê$²;üÛ]?Áiànj?ó0¥i±t'@¥Ðȯܧ?ï,pk¢æI¿æÌs 3&H¿åM÷¤ç«u¿évØa´P¿ïÿáåÔ?ïþø™q¥UNASNone?ïí@ŠK?ak×d¹f¶?b¿=wË?ak×d¹f¶?ïÅOU†Lé?‡d.ëµL&?}XU@I'Y?‡d.ëµL&?ïj"Ё.¶?ˆÿ0þ	?'¯e겿D?ˆÿ0þ	?ï"hx ‹â?uH†	¤ƒ?Žåá×Ýi?uH†	¤ƒ?ïoÞï(F?"UÝ{G~W?'"nó+?"UÝ{G~W?ìü_xÓ¸?Àr'^W'þ?¸D§UÃ?Àr'^W'þ?í81<c·?§\ç`eµ?¶>vUµÆ?§\ç`eµ?꣥ØÛè?¯ÿÐtëòÿ?Åqhœ]Ê?¯ÿÐtëòÿAGN4FGL J0058.3-4603¿æ£"K™ÀQÁqKœ¶…À;µÀ_@˜À=BûÅ@ô*û×&m?ÿZÊ¡yaì?Ú¢w{?© ÷œY<‡?ÊYƒ©î%@YÅM~¹?ïaì¹ÒE¿ëlÎàM]+¿Î	m&žû-¿ÜSa[ºà¿åG®záH¿¬U½KÐcUNASNone?ïÿp*µ`J?	>Ý(É?ú¯rüð,?	>Ý(É?ï÷-žì?TR3-ÜÚ?Qý¤;w:?TR3-ÜÚ?ïø¸Çöèï?W˜Þ'Mù;?Mßçã$ç?W˜Þ'Mù;?ïÿ›ÒP?Úí¶Ñ¬?^îW=á?Úí¶Ñ¬?ïÿ·dtŠ>ýûr°¤€Ô?&çå>W>ýûr°¤€Ô?ïېu"½Î?xÓWmxº?r7Å#5&?xÓWmxº?ïû
‰^?\RDåôü?CïÊbގ³?\RDåôü?ïýœW±d3?' MçaG?3A/iÐD?' MçaGAGN4FGL J0059.4-5654?äÐó¹†ÛÀN°ËæÀ9¹Â^´Á=À<êAQÚ@vr€ó@¢ÈY …F?³K¯ÁN>|?É·¾]HZ@Ú­Å@§Ó"ý0¿Ê]%Ÿ÷¬Ÿ¿á¬M P¿ænij&å¿ê–a¡Çæ¿ì6ÎÉ&O¿ïûÛxa:­UNASNone3FGL J0059.1-5701?ïÀÊApý]?zé!tÍe?šß/t
£?zé!tÍe?ïîHÏk|j?dñ€öáy|?a·0"vu?dñ€öáy|?ïn[øÑ?…î%:‹¼î?'0{Õ;ñ?…î%:‹¼î?ïàûHhØ?Sâ‡PÄ!-?o·SϚ?Sâ‡PÄ!-?íßÐò:3q?®_éÌA?±xn.du?®_éÌA?ï¸T_¨²?"oìˆ:1æ?êè!ÚØ?"oìˆ:1æ?é嬘,´?³óè?èúà?ÈiMŸMÁ2?³óè?èúà?îÉLMœ§&?'7Õ²¹ )?£k;!ê
 ?'7Õ²¹ )AGN4FGL J0102.0-6240?çk]QûÜkÀK3¡fµÀ;eTÑél@À<à£ó¯5@ N:¶?ý»ed®?Ët˜Ù*S;?¸½ÔakªÉ?ðuøÅyu@*AeûÝ\?ìö—€º¦?ÔüÍÛëx´¿Ú}âïN¿ÚÁ1æ,¿æÕ)' ¿É :Š¿âUNASNone?ïÿyó¿ˆt?qÌ;j¥Ã?Á
¿É+?qÌ;j¥Ã?ïö~Ba_¨?SÝðb]€)?S{Jÿ À?SÝðb]€)?ïöD&9ir?`×B¤nό?Sw³{,»?`×B¤nό?ïúw
V"Õ?.&g.@à?F#֞" ?.&g.@à?ïÿƒu뿁?Ɏ&m2«?"Š*Wø…?Ɏ&m2«?ïÚJ×>À°?|N›Äl+?rڔtcà?|N›Äl+?ïø/)kç¸?b*$Ç*»†?OCZ&U©?b*$Ç*»†?ïð]Ì k?M¥ÕÜOՋ?_Dgyð?M¥ÕÜOՋAGN4FGL J0102.1+4458?ç¹+¿îºÀ1ܬ¯öÓ1À;@e+ÓÃÀ<®Ó5œš@ )çJ?í)•€r+?ݾ¬
9¤f?ëìjŒeÔp@<¥¢¼@¡¶É€<%¿ï£'Á¹m?áÎϦ›àœ¿éçzBfV÷¿§k®yÐ{ƒ¿âXxgꍿïús™TÐ<UNASNone3FGL J0102.1+4458?ïø¥,Â"F?HÎ;×°wJ?MkLûÜÍ??HÎ;×°wJ?ïíÊ?Ì9?g4;qGLd?b5ÀnÜ?g4;qGLd?ï¢×ʘ?|}'jˆ?‡J
tš¢&?|}'jˆ?ïÙןlÓ?_Ìe|d27?s|Êk?_Ìe|d27?ïܬ'Ë`?s'NŽ±Èµ?q©¾ã|§ö?s'NŽ±Èµ?ïµ¼ä2«4?OâÃ
™?'ÇÀâ?OâÃ
™?ï^'gw?±<ò{gg?"/³a2?±<ò{gg?︇Bx©?{ÿoõÐãó?Þ?ê'aÂ?{ÿoõÐãóAGN4FGL J0102.3+1000¿ÄA1RÀJaä¼­šØÀ:µ¸•Þ#6À<aÁLf
@ œ¢»×1*?ùÙú—á2µ?Ò[ÈRèÛ?Ú³ô#Rë_@˜Cæߞ?ýqÆ^s¨Ä¿Û®ž#/—¿ïÄÜ"«%³?íûÀ«+g¿Ò†É]VF¿æ4½vît¿ä íìEzUNASNone?ïø…pÓãÔ?Fb"ißÍh?Mê;«Û ?Fb"ißÍh?ïÒO;/3¨?+g.YÑû?vØbˆ²è?+g.YÑû?jÂ
#?†GVôk?Œ™¥A¾Gk?†GVôk?î÷SzÅí?ˆG9¯¥? ŠÈ`ûo,?ˆG9¯¥?ïï>Ê7u?]ü"»ˆ!7?`Á5ßÉËY?]ü"»ˆ!7?ïa'õ™'a? 8ªØG?"Í¡N'áÏ? 8ªØG?ï\>2g"?'jÔÁ*/¾?"x9µsãÔ?'jÔÁ*/¾?ìéI(Ä?ª(>vS›?¸·¶jÒà?ª(>vS›AGN4FGL J0104.6-0818?à$õº_jÀQ»<`ŸÀ;	7·&rÀ<ƒM#ŸA@/x›æ@¡Ñv€?Ö ¡`7x<?µ¶|~UÆ[?àˆÅ †l@½6	Í¿­g:f¿í»Ó`Þj¿Âe?	U>¿äÉùHUÚ'¿ïÿîͨ"ß?ïž^z^ÁUNASNone?ïùqn_âœ?[Uÿ¶»Ò?J:F"³^»?[Uÿ¶»Ò?ïïvRö$¾?d¥Ž3GG?`‰­ùŠi?d¥Ž3GG?ïV$¡
ðó?ŒË 0iWÇ?•;kÚÒEž?ŒË 0iWÇ?ïøOd—.Z?<P¤§œ¹B?NÂn¡CNË?<P¤§œ¹B?ïúñ½
ü¢?J ¢ã<à?D9–Ø?J ¢ã<à?ïºë²ñ|?ªõG=?E:šVü?ªõG=?ï‡2¾–]?ŽœÑ°¬ó£?Ž3P_J´?ŽœÑ°¬ó£?ïÑ\,ë_N?m/Àjœ_?wQép3Q6?m/Àjœ_AGN4FGL J0106.1+1131¿ïÐLX?©†ÀI–áïsÀÂÀ;ez¤£À<ºÓø:9@ [ž·:¿?ý$™ù;?Ò;9\B 6?ÐX9™…x?ùO¡(TH@ç`Õ®?ë<7Þé"é¿ïþôœõn­?ïóeRj0 ¿èä‡Ôu7»¿Æek"£'¿ðUNASNone?ïþCÔãi?&_³Zê%?+´‰Î(?&_³Zê%?ïò©¹³{©?^ú÷"™þ?Z¬Œ_O=ü?^ú÷"™þ?ïÏ\ü8?w˜\³Z?xpÑ¢=7ß?w˜\³Z?ïùGnuöÊ?9]›3_‡Ï?JâEü¶–ª?9]›3_‡Ï?ïþA+ð…?)ãÏ& IK?+íO¾\{?)ãÏ& IK?ïÊ­i@q›?ÙYÎT˜¨?z©KHiÚq?ÙYÎT˜¨?ï®l Svc?"ñþ¾*ã?"d÷ûø}?"ñþ¾*ã?ïñbT¢³c?V)3'˜
[?];W.Q?V)3'˜
[AGN4FGL J0112.0+3442¿ÞU¸€†ðlÀ;úÞ]	À;/6oþ•À<µS,;d@Q#RŸÊ?ÿ×_f˜?ÙüxŒØ"?Þáp}–ƒ»?üÞΌÀmC@
?ىʿî´¡'¢?クAûM¿ÞÙ§{¯xÔ¿ä ‹Ær?¸¿ïÿ«çy÷=?ïüK_ÏÉVUNASNone?ïëQ¬gt?rÝþ¡¦Æb?db®Yëþ?rÝþ¡¦Æb?ïé{2•n?kð7Ò&˜c?f"Í~&bG?kð7Ò&˜c?îuŽJíd?•)ME¯?¨§R	ðÁ?•)ME¯?ïÀäÎÔa?hm"ì^Ð?˜Y‡?hm"ì^Ð?ï¸"üYW_?§ÿg•'?÷@ÝKC?§ÿg•'?ïFаq?š¶s,
L?%ãÙö?š¶s,
L?í|¾—ä?£¿vÝ]çÝ?·D±ô`?£¿vÝ]çÝ?î¡
±VF*?—Ý®ÇS;;?¥ïTèèa?—Ý®ÇS;;AGN4FGL J0115.4-2917¿á²bigßÀUvÈ´9XÀ;‡ÚÙÖÀ<äÔÉ'@ µQù#?ûûI·Ùö?Ֆ¬Ÿ…ÁË?Âß#¼r·ƒ?ðZ%Ðt!@Û¨!Ç¥ñ¿ïÿC*!<?ïéÿºùf¿çÀèÞ%d¾¿·½WÓ{"¿ÔÝ[û©Y*¿èÏ^bùUNASNone?ïÿ…@
 ?à0äsLš?/^rݟ?à0äsLš?ïó´ÇaAÓ?^óä¬Gà?X–p¿
ºj?^óä¬Gà?ï¬ÿt?[ÍÐ
2ì?`cx/D›Ð?[ÍÐ
2ì?ïýï•,U&?£'kG<?0ƒVa÷(–?£'kG<?ïþ¼8ù5? X*
N0‡?$<yµÜe? X*
N0‡?ïψŒ²?€34%o§ã?x;±Jۂ?€34%o§ã?ïéG©"?¸?p£eÃ_?f¸VG†8«?p£eÃ_?ï÷"8­?Jý~ÎÍlß?Q»X
5Z?Jý~ÎÍlßAGN4FGL J0116.8+6914?ì{b]±ûª@ì !sOÀ:Eûg¿,À;Ó2ӑâì@®Gp­@=Û	íÀ?Ò`¡üi?éÃãŸw),@Š˜í¢/j?ôå~I‡¿áWR'ú¿ÞHTbWãí¿éÜG^cb¦¿ïýÅÞFî¿ë~Ïu¿â©¬ ÚÁUNASNone3FGL J0116.8+6913?é¼a«Ò½?Ëo4<ö¼?ËÁyPµ
?Ëo4<ö¼?ÊÂïqp
b?Å"¤ÿ˜ù?éOD#£ü¨?Å"¤ÿ˜ù?çÛë6«só?®·"ä$·'?ÐH)'©?®·"ä$·'?ʳYÜó¿?­û£ÛÚ	?éS)ˆÃ>?­û£ÛÚ	?ڙC¾û?Ò"â N²ž?â³^xu '?Ò"â N²ž?™®é%â¬w?£Q2À¥)Î?ï2ˆ¶Ðêœ?£Q2À¥)Î?ڊ#¡è?¹€Ý)Và?âºî/õñ?¹€Ý)Và?r—KÐQÖP?eä@Wih?ïÚÑh¤$?eä@WihMIXED4FGL J0118.3-6008?¥´Šê1ëÀLUA [ÀÀ;Ëô_¹À<Üò@úœ@¹±Y¤·@&Š"lXï?ʇSÆы#?Ǖb¨@ÑV?ü°Í'eŸ—@m-Dܨã¿ï"Eg]Ñ?ïÆlËÛ5E¿áÅ|vs#ä¿àހ("Y¿êͶ±Æa¿ïÿ¼®q—óUNASNone?ïûu{Ï{ ?@CÛÍ|š?B*ê3U?@CÛÍ|š?ïö­­•?SáæÇÅ0?R¤¦U{Dâ?SáæÇÅ0?ïÁõ4í??v¿úO;¥f?elƒÈ_?v¿úO;¥f?ïû¼
K¢/?+
´Ÿâ~?A×­^D?+
´Ÿâ~?ïû'¥Ø¹Œ?D•!–èF?CagÑ°ïD?D•!–èF?ïÙòF¦O?yôð—:?sܔË;™?yôð—:?ï`é×ʁÄ?^"ƒÝæ?"âň]‹?^"ƒÝæ?ïòÚ[¼Ðg?PŽŽÁ€ë±?ZKHuáà?PŽŽÁ€ë±AGN4FGL J0120.1+0505¿Þ»¥ ûÀL…£~õ©À;1bZh+cÀ<aG¾Ûr'@Uë²;|@ÿí¦a(9?Äõ¹NjÇ¿¸¼öëÚ.?òÑ8×·âZ@¨«B8‰´¿Á1³VY(¿íáqŸ¿á_ã*cǿ⼫™Ÿ¿çª£	"¾¿ïÿ¤DîUNASNone?ïî!'þï×?¢ë\Çóð?aÞ|Î5ñ<?¢ë\Çóð?ïð;‰:s;?b¾<î ?§?_ˆíYŸ*–?b¾<î ?§?ïæ¸*ÿ2%?r,µôô'?iGÔßћm?r,µôô'?ïù×ëAŠ—?2´S+ÖøÚ?H Rjåâ×?2´S+ÖøÚ?ïü¹Ë#?6
鍂¨Ò?:1¥ˆ	o ?6
鍂¨Ò?ﵫ·Ã?'Ø{ÔÒÊ?~¥*
q

?'Ø{ÔÒÊ?ïρÔÅ®d?~˜ í˜@Ë?x?µåý»?~˜ í˜@Ë?ï¾q=Áê?sØpüåÁØ?€c°"ƒ‰?sØpüåÁØAGN4FGL J0120.2-7944?îÚÑ4€kÀB¦>-b9À:ÛWvšÙÀ<-"¶³…Ô@L>7±@®åD'×?ÃЀ¶sÄô¿·gɽέ"?øʶ!œÁ@BÏÁ+?ïÖ%œq»¿ê>
A¢a¿¿äè%þÂ=R¿écÑÌk¿ÊÉ>!ù¤ò¿ã+ÕÁh¼UNASNone?ïþè"
8`?ȁ}!*?!}â`Uv?ȁ}!*?ïô3Ć4ë?Z('ÃÞ"ø?W˜v®Ýùp?Z('ÃÞ"ø?ïîbÓM´-?b7"á–Zb?a,·Ë3G?b7"á–Zb?ïþ<´ÿ?áo»Ìj?,7ë
Š>î?áo»Ìj?ïþð±Œ=?#Gcñ
…? ôès(5?#Gcñ
…?ïΗ¢Én?&ډ÷®®?x´.ž¸1?&ډ÷®®?ïÊhz×{k?~2{‹
P%?z˦Ð.A?~2{‹
P%?ïåΣ¼ˆ1?di@
ž½ˆ?j1\YuNÐ?di@
ž½ˆAGN4FGL J0122.4+1034¿ï¤ªUáVÀIÇ:Þ"_¦À;—KÔèëÀ<È[Q_n%@"5Ï`ûÃZ?÷{Ãà•®?ÔÔÈ#š¹Õ?Ôwã¼R?ÿC;¾òïv@aƒ~ûÉ¿ë-Óî'¿ïÿÿ>¹ú?ïÿç@ìYZ?Ô1ÄPÈÅ¿Ýbí`>¿ÖöçþV‡¡UNASNone?ïý×w(^!?%õ¥Q¿?1DFxãˆ?%õ¥Q¿?ïòƒK8Ã?^+>"a"m?Zùj:š?^+>"a"m?ïà8C,>f?mA¦dÂp'?oǼ½Äî?mA¦dÂp'?ïøÏâ«Ü<?>LÙqt?LÀuûˆj†?>LÙqt?ïþnÄȋ8?$'§ë‡<^?)¶ÍB?$'§ë‡<^?ïʾ—LYÂ?':œuwi"?z ´P46ó?':œuwi"?ïñ#¯:HY?eå#ŽX%?]¸¡g³^b?eå#ŽX%?ïï2Ay·?[žz•¤—Ñ?`ÍéyΠ?[žz•¤—ÑAGN4FGL J0125.3+6820?í|q+Ö@³çÑ5ZÀ9ÛîùûÀ;x¡L'H@¥§Yޙ@´hqH?ÓL.!%"?Ðü^ØP@¼½‹j@&¼<
L?ïÙº`ú?ÎGŸ{ÛË¿ê×2K¬¦½¿åÁ'¶ÿ.¿èЩôg¿ïüuÁù	AUNASNone?ï6²,žª·?œ²ñÚMhé?™)ºqR"?œ²ñÚMhé?ë؀ÅÀǎ?¼Ç4X˜?ÀüèüáÆ?¼Ç4X˜?î̓ÎM£?œ¬êBú1§?®"'ÄÒóÑ?œ¬êBú1§?ëŒ/–ψ? -Dÿú³?ÁÏA¤Ã¡Þ? -Dÿú³?á2f´ahr?ÎÌ]] '?ݛ2—=/?ÎÌ]] '?ØeäEVJ?Òåå1Èz?ãÍ
Ý8TÛ?Òåå1Èz?ᮋ&]?»-˜½âµ?Ü£Æé³ãG?»-˜½âµ?Ï•,¼:r?´'õìŒ?è;´Ðñc?´'õìŒMIXED4FGL J0125.9-6303?àn\XèÆËÀJÐ\
V›À;D}¿H€À<Þ\)̂$@¡·â@ǧ¡š?Æ®^øˆèF?•ECV1?ѧa5úä@•èÞ%?샮uɱ¿â/-êôÖ¿è"·õ¥3+¿ÜCÄûÈõ¿å Ž¶È¥¿ÝVÁÃ.hsUNASNone?ïý«MPÒ?$žkO)??2£{Â."Z?$žkO)??ïõ³ƒK?U±5B<?T˜åøê7?U±5B<?ïóe›÷S?SǺj§Å(?Y4È,Ö­?SǺj§Å(?ïû¦uäÍc?%úbsŒ]ð?Af(òa¨?%úbsŒ]ð?ïý¢z2T?*ŸÝOÉÕ?2ï+Á"\?*ŸÝOÉÕ?ï×Ú1©	?~ÁMéö?tw'Þ<n?~ÁMéö?ïõË¡S¢??`öœ{4¢t?Th¼Ò
Ó³?`öœ{4¢t?ïë¼°0E(?RÒ»ô?[û?dCO»/¸?RÒ»ô?[ûAGN4FGL J0126.3-6746¿ëp\BpïÀHJä)à¤À<D'À=-®Õߛ@!óhbêÛÖ?÷Æ5µ?ÚZâ9E›ì?҆êCM?÷ĞDú?û/,xƒõC¿ïþ…A¿êvjXŠÜ?ïûÚÂXÖ?À{ÝÆðú¿íƒ>Ò£¦?è	K¾DsÍUNASNone?ïòn=å¼?_¹]£Ûý?[#ƒÕÇy$?_¹]£Ûý?ïó:ý#y#?\Ÿ3|¦9%?YŠ4¿¨·?\Ÿ3|¦9%?î¶m™zSÈ?–µDzßü?¤™&l¦F{?–µDzßü?ïë|£a'?Y"з}K?dƒæI`Ÿ:?Y"з}K?ïõý};s?]ÓïUã·J?TúÜMÊî?]ÓïUã·J?ïѓ
Áè ?€6–éñâ?w6y4Yƒì?€6–éñâ?ï2âiRe9?":üøá?™£²ÒC¼ë?":üøá?ï¾àb´^?}Ñ¢Vÿ?€Gä;B'?}Ñ¢VÿAGN4FGL J0126.8+2412?Õp†c9"ÓÀBú€If{_À:4ÿ—$tTÀ<EÔº.@£øÿ%@ƒCÿF?¼®î?Ž5b¿~áè÷¤<?³ðëºù'@êt¼•r¿ß^E"^ǿ䢅›µÓŒ¿èLÒJ»¿ì(S 8"¬¿Ò`P'yl~¿ïþÁÁÖυUNASNone?ïÆI9s­æ?±CR=¤ <?|Ûc?ùÀÐ?±CR=¤ <?ïõk'}Ï?X>¢ð2í
?U(ÛwÔ²¨?X>¢ð2í
?ïß=há?~©p˜Á?pazc\g}?~©p˜Á?ïÿ›],ð">ùQŒýuƁ?	(Äuéx	>ùQŒýuƁ?ïÿe"•‰ü? ˆ«ÒMÚ¿?Msúã? ˆ«ÒMÚ¿?ïÕâ=Tý¼?z§Ï§D•m?uátmå?z§Ï§D•m?ïæÙÙz°?t²´ôšr?iû&G³?t²´ôšr?ïþÛÄG©?%dc_"'?."F{5g­?%dc_"'AGN4FGL J0128.1+7542?íEò®fbé@)ÿ]5e<›À;,$8Äl¬À<žÏœŠå¢@W­~'ù@cYÿOÖØ?؉$Vv"?îš#A΁ƒ@þÚH¶R@ݲ"L*{¿ï‹oÀbV?ïâù)L)¤¿Ü¤K8ãv\¿í8"†<Ń¿ïþ¯çÜô?íHúåäËÇUNASNone?ï/ՀO›Ÿ? š³Å·&?šOòœð/? š³Å·&?ê'ûž"Ì?Ęûє ?Å÷Ü…°Ñ?Ęûє ?샳U¨‡?¢'5 _Q?»âgåR»Ë?¢'5 _Q?é<]—›ù¬?¯ˆÎ
ނ?ˉ¡N?¯ˆÎ
ނ?êâòi¥œB?Å[ûz‰?Ät6YiŽö?Å[ûz‰?Ì'7
™'?ÌãŽ<:»4?èÿ_r<™ ?ÌãŽ<:»4?äu¶ç÷åC?º2Ñl!nî?×'05z?º2Ñl!nî?ȅðå…ÖC?²ÌüEhóg?éރƞŠo?²ÌüEhógMIXED4FGL J0131.7-5346?àw½FÀO*êt}€^À:¿¾Ô¼…WÀ<µâ;ÉÚª@œ,Œ@6&˜ðý?Ñï ´«m×?ќã›EkD?ú:¹¤ÑÜ@×'n®ß¿ÕLýԺؿß]"Y¿ÜYãÜþ¿éâç¡'û¿é,Š'O{¿ 'ðpUNASNone3FGL J0132.1-5340?ïï8Hè–?[É<­&?`Ç÷†üâS?[É<­&?ïïV
ß¾?h×ñCý˜?`ó©ÇÅj?h×ñCý˜?ïhœ"Ç?†tOƒ?'ÿ¬¹ê?†tOƒ?ïä˜ö(R?TùðýE?kg	ÒyMŒ?TùðýE?ïºä0Á"?}ôa
æɲ?†ä±S?}ôa
æɲ?ï¹èCNH?Œ¤¹¿F)ð?…ïD{B?Œ¤¹¿F)ð?탤o
Ä?¡‹Õۛ?³â܉§_à?¡‹Õۛ?ïg»\çô?"ƒÊVN6?"Ÿœú?"ƒÊVN6AGN4FGL J0132.1-0956¿ïäê{^pÀQ"KâCÀ:>_ïSàÀ<]o`
+Ó@¯Ûbç«Ë@'¤:Œ?²äôQ ?Ô.;&Ǖ@TbeOåñ@	šhÓ(0¡¿×Ŕ~ýŒ¿åŒqȚ8%¿ì†ƒý¦"¿éS>Ïu¿îáGB´°v¿ïóímVD°UNASNone?ïîwî_Tà?b>5¬g?aˆŒ
w´?b>5¬g?ïçI—<‹æ?sD5é¸Â1?h¶h½ô¹Æ?sD5é¸Â1?îé]A#¶¾?–Héi?Ӎ?¡j+íĔ?–Héi?Ӎ?ïÛ€ðo-?[
|JžGË?rw¿sÚ­Š?[
|JžGË?ïìÖP•Tø?d9‹·b¾?c)¯"æX7?d9‹·b¾?ï'Sï?•BŸÊ¦¥ó?‹¾k0Éq?•BŸÊ¦¥ó?î¯;Vî#_?™ùÃÉð"?¥J'ù±?™ùÃÉð"?*"yŽ?• Eª?§Ý]Øg$?• EªAGN4FGL J0133.0+5931¿ê'Oâb؊ÀP!p"À:Æ(Oªb?À;Ó	¢z@ -Zk[mº@ëùŒHx?Âcwž™¿µ§â1¸ß°?õÄÒG`â?þ-°€0?îIDíoڃ¿êd%¿]"¿êŒ77…¨¿äãÉª¿ÝÖt{'H¿Ä™¢}îÃBUNASNone3FGL J0133.3+5930?ïöŠuˆ?zÄÖÇ?RëÀØuÁ?zÄÖÇ?ïʈo?ƒ †0:˜?zõ»ÛoFD?ƒ †0:˜?ï°ÕþØ@Q?'þÂ%D;?ƒÊ€<ágÐ?'þÂ%D;?ï×wWQ?a~Úçg?tDTöe¼?a~Úçg?ïÁ"Ì«S?BnNç?n™±YŽC?BnNç?í°<L¦:¬?º}Û«•x*?²~šÎ*£?º}Û«•x*?ï'L¸ëD?"l(-Ô'?›–lR3‹?"l(-Ô'?í]Œã}¾G?©I
QVœµ?µ˜åÉÛÇ?©I
QVœµAGN4FGL J0137.3-3239?îUowuòÀS§ÃÞ灄À;eEW"&À<Ízí(@']gå@àâ-‡"?ÑB	D¢Ff?ÈÕd.'Ü?ó^"ð•)@sÔ
ƒ¼Ž¿ï‰µ@>3—?ï1g`âC¿é<6a»Ü»¿Ì÷iCŸ/¿ð?ïÿÿ" 5•UNASNone?ï¼yïk?©U;ÑÕYÀ?€ý8Ô«7?©U;ÑÕYÀ?ïñÎÊ0™?ehžqY?]øbÑS=Ã?ehžqY?ïñÇFêº?"ƒ0'=?œAÇû>Ë?"ƒ0'=?ïøŒ©Ï¥M?=—^ÈîfÇ?MÍWàm¾?=—^ÈîfÇ?ïb'
å?¡Ð*WõèØ?"­¾7àKm?¡Ð*WõèØ?ïµsø`î?)X
zy»?'£õÀ
m?)X
zy»?î²ÍÙDÞ?˜áÀrøû<?¤Þü'?˜áÀrøû<?¦ƒ§ ?výA
VIÍ?€ßDe‹þ?výA
VIÍAGN4FGL J0138.5+0300?ãÝO=âÀLåùð†nÀ;h¯Á#K_À<¾eò£ +@ "ÆÎ1@^	}?Í[PޔËT?ƒu¤5à?«Þˆ6íg@jÒ/6_¿ïÿÿ" 5•?ïÿþó…õ¿á´ò…Ãù¿¿Ô8ؤ}µ¿êD°~b†ˆ?¶²
>GclUNASNone?ïûƒËjæÃ?AP
ÃƞQ?AðҚ6Ÿ ?AP
ÃƞQ?ïòo'*"?b³œ<¨e?[û!"'Z×?b³œ<¨e?ï‰g§mË?‹Ñ–—"õ7?¦8 sa"?‹Ñ–—"õ7?ïùx-|ÿŸ?43<Ҋ?JKVƚ?43<Ҋ?ïû§A«z?A7æhF.?CåcñÏqÇ?A7æhF.?ïÊ"=ö
l?Œ!%/Š•?zîàê,Ve?Œ!%/Š•?ï XÝ^7?{¤þ"?Œ7éχª=?{¤þ"?ïãïgÃ2?a¬ªVd?l™˜å¦?a¬ªVdAGN4FGL J0139.5-2228¿äô~•îOÀSˆtÀœ<âÀ;G-½¨l›À=, ñèH@ÃÞ,ñz¬?øõΞ^$y?Ò ì¹ý?ìÜB 6m@"ÿßHÐ@GYþí¿ïÿtõubƒ?ïöû¿©xµ¿Ë¨qx¾¿ÞÇlüÃ¥¿înX}šŠ…¿ïþœÞGžzUNASNone?à¨öšëB?АX
›\?Þ®Ê){Ç?АX
›\?êªò®¢"?ÇÈwÆO?ÅT5Euïµ?ÇÈwÆO?àóÚÎuÌé?´0ÅÕ¿Á?ÞJcf-?´0ÅÕ¿Á?é?1ib!ç?®öU'õx?Ë:Zwxe?®öU'õx?ÍÝ:|Âb*?É¿Ò¤ŽP?舱`Ïgv?É¿Ò¤ŽP?ß80¦™?ÔWaWÖ"-?à{ã笳8?ÔWaWÖ"-?ÖVŸJä?µ'W~1­N?äÔ°Zóù?µ'W~1­N?ÚÒ¨©ï?ÂjÙ>ís?▫«?~?ÂjÙ>ísMIXED4FGL J0140.3+7054?Ò#Åô㹛@ ÔFQóè›À:ÒIì³"À<k{µƒ@!+µg*†'?ûÑòkyÌ?Ϋæã¤T´?Ç3÷©D\{?ôG÷EF[.@ÄøÂôÝ?æ¹úݬC¿é"³ì+6å¿ãËgÝ^ëH¿Ô§ÿê8î¿ÙÓ¡šÀ`¿áP1ZëßUNASNone?ïûºÑÖ) ?5!«Îfá?A¸þÂÁ?5!«Îfá?ïç¯î	v?h¥üÍM}?hPûש?h¥üÍM}?ïéÆËÞ?^˜†J¡Å?fì9+G9ü?^˜†J¡Å?ïÖ]Ó«õM?T·C
B¿?tÑ
؍¥?T·C
B¿?ïû{|Uċ?9^V¬H7?B×=e?9^V¬H7?ïk ·ðòœ?–¼"';º?'‹èþrˆ?–¼"';º?ïÚûÚ_8?vÙå͙bR?r'ÕGØ?vÙå͙bR?ï6ҜfõÐ?"1&$ï.?™%¬{¸Kû?"1&$ï.AGN4FGL J0140.5-4730¿Ð77g}ñ%ÀPÞ]öU\À;ÚVùÀ<¦RFñƒ@ªÅZ'§@<Ö!à$˜?Ô4›þxÁ]?Ã6«¸«Ì?è;†ß؝@ðš$W"¿çñ¦¿òÊ¿å…Âýk%=¿ãhN}¼n[¿èãX_<¦¿ïú
!ыù¿ï&Nyà—UNASNone?ïý²$wP?P¢ß¼\Gð?2nܾq¿/?P¢ß¼\Gð?ïõ^lÙv?[úûz/?UC%Ċ³ù?[úûz/?ïÒHt?uˆ<X¯œK?vÛÅâòƒä?uˆ<X¯œK?ïú¢¶¬W•?1'Iv‰Fû?Eu$¹v?1'Iv‰Fû?ïú;**e?L¹Ý›võr?GçD¥YÊ?L¹Ý›võr?ïÖ@י?{±~íbÆ?tßô–ó%—?{±~íbÆ?ï¢ò¢Ž#³?ˆºŽ‹ècÔ?‡CWN¸£4?ˆºŽ‹ècÔ?ï㾍2ÇÂ?`ÁÅiw"?lArÕwMº?`ÁÅiw"AGN4FGL J0142.5+6650¿äŸ[žûòï@Ö¬¸ZOÀ:Y§uû.àÀ;nŽ	Bžá@¨³0C"ª@,ʦßi?âä"wy3?âHȐýé¥@¶B9`sÞ@z;×F£R¿êÕb{uA¿Ž oPÅ»¿ç†è‡=vƒ¿ël°Í'Åj¿ç#Ÿ!BðÀ¿ïÿ¥œÝùUNASNone?î3à'Úì(?¹Œj¤ª?¬ÁöÔäò~?¹Œj¤ª?鐌=¡²S?ÆÞ)á¥ÌÙ?ɽÏ	y6´?ÆÞ)á¥ÌÙ?ì÷ÊMŸ#?¤ç¸_¨=>?¸Cñ¯JÔç?¤ç¸_¨=>?ퟠUÒ? .Mil	¦?·Ûü{êq? .Mil	¦?èHççô?̦8C=lr?ÎÜc"`/ý?̦8C=lr?Ë.>tã_i?Î¥SvŸ™Ž?é4pbÇ(&?Î¥SvŸ™Ž?ãW"$ü(?½iß A²?ÙP÷ñ¶±?½iß A²?Ðu÷Ø-þ?½<^'A²?çÅét?½<^'A²MIXED4FGL J0144.3+5959¿èw»½¨9À"%B{¦À9Ýv<?AÀ;ŒjýŒˆ@:/&‰+¸@ŒÍ{Hu»?ůŸ)üRÌ?³yéûÜ°?ç@#qPM@J')ÞuÂ?恋ñ:j_¿–ƒaô¼ªì¿çÓ¦¹Ù«¿ëg¾Ö¿èR¬?Ž‹I¿ïúK¹ëUNASNone?ïù&QÎSà?Jl»R鷂?Kf¸ì•|?Jl»R鷂?ïÖOΰã? Z£Bšn?tØž&"? Z£Bšn?ïrÕ)膽?‡LcT6?'¥ZÆ^Äh?‡LcT6?ÎÔ ?mPF´‹q?‰ÙÌX–k¨?mPF´‹q?ïÑæbÜ)r?}†œA_µä?wÎ{íÆö?}†œA_µä?ïu"@òŽ?©a'P:¥Ï?Ÿq[·á®0?©a'P:¥Ï?í_LáQ‹…?¤£Yò×J?µ˜õs£Õ?¤£Yò×J?ìÿ4ó¥?Ÿ±õÏÞ!?¸XgÀƔ?Ÿ±õÏÞ!	AGN4FGL J0150.4+4848?䶈µ=À)֊"lXïÀ;•PÔ-êÀ=5²Ñyø@ ÔYM= ?û?ƒ¾f½?Ö19'ò¹?ïöá=@K¡¿	?õ›?¤Á?ïÿFÄ¾¿é9M(¨¿âšýFè?ÎuÎù¢Ãº¿ì
îÛëMÁ¿ðUNASNone3FGL J0149.6+4846?éI½—ê[Ã?Ç~ƒ•Ã˜"?ÊÙ	 Võ?Ç~ƒ•Ã˜"?àç…e¸Ÿ!?Î	ßÎmr?Þ0õ4ŽÁ¾?Î	ßÎmr?éHß>-Q?¯@ó5í?Ê܃J»Õ?¯@ó5í?وPZz8Å?¶*çÈò9Ó?ã;×ÒÂã?¶*çÈò9Ó?éN±žŸí?ÊWÛ9³;<?ÊÅ9‡­€N?ÊWÛ9³;<?Á¿|yš˜?ÄXÁq=É©?ë á™Yû?ÄXÁq=É©?⸰"û‹/?º(K£—?ڎŸºé¢?º(K£—?´MÝèlÕ/?§ö´6Yׂ?ívDB­­*?§ö´6YׂMIXED4FGL J0150.9+1230?î`fF¨RfÀGè>ÕÀ;LK?™sÀ<‡ñS"ÒŠ@ZEÚ)ו@U×DõÓV?ˆ#›»_?¡»
²›R?×W"%ĵ§@Ù¡œrg¿âg¨mqó¿ß
º¨²ç¿çÜ7Hkª¿ä›…AÚ¿ÑYƒÅœØ¿ïÿ`h¤
UNASNone?ïþ"	÷>?$…¸?&ÏaØ%~_?$…¸?ïô; ðîô?[ɶàCÈ?W‰¾J‹?[ɶàCÈ?ïñ×ÈJ8?a;³è€Ù™?\Pp<Ÿ^Ó?a;³è€Ù™?ïþÚûÛû`?+¯PtËÅ?"PAW1H¹?+¯PtËÅ?ïþ·by¿+?©qûør?$‰Ù¿f?©qûør?ïѯÓ}ý?\(i'€?w}'ÿ"•"?\(i'€?ïæ©åÓ?sâ·…*Ø?iVé.ü»?sâ·…*Ø?ïøˆïÔ?GXÞ҉?OÛ–å4?GXÞ҉AGN4FGL J0153.3+5416?ïþ&•¯ÃìÀ	/+f¶À:êo.Œ†À<‹ú©u°@!"6s?þÌœ†³ä?ċÕ`ÅÂ?"oŒ™šµ?ÐGÖ"¶ä-@íîò;œ8¿â'^⎀¿ãvÍòfºI¿äÊÄ°ž™¿ÛþüôâÀ¿âÉUê`o¿Ïu6
GUNASNone?ïÿ	µW݄?ò§¥ÒÈ?ÉLÛ='?ò§¥ÒÈ?ïóäÐh|…?^ኪV•å?X6^òÖ_?^ኪV•å?ïõ™CÕº)?mØ­‡3yÎ?TÍwáÏQ?mØ­‡3yÎ?ïû;mœï?*Â/'ñž?CIEX€{?*Â/'ñž?ïÿ2 .?ÂðáPM?­ùU+[›?ÂðáPM?ïÃÔv&ù?‹ô™;ó²?~þ΋k"?‹ô™;ó²?ïò]/2â?sà}½rÍ4?[Eó hì+?sà}½rÍ4?ï옚Iî?T^X'á?cgáe¶K?T^X'áAGN4FGL J0154.6+0051¿ïôÜêëà}ÀMÄq´xBÀ;ÆÙ{0øÆÀ<É·sŸ4
@!³uy/A?ß¡ª	SeÙ?è«@UZ¥h?ïäNÿA"?ü}å#çÆ@†?`"¿áýÞ½ç¿ïÿ<h"?ïÒ¯´ì¿æÖÿöÅě?ÎÌc8°¿ïÍ­ÓïUNASNone?ïù ïØ?Fð ÇVïù?H÷€ivŠÙ?Fð ÇVïù?ïópß«?]kˆÒ‰?XáÚÔ	ž?]kˆÒ‰?ïuáëºE-?…ß"ô첎?'CŒ&öV?…ß"ô첎?ïûµßå>?7Ì
T[J[?A(î6ãS?7Ì
T[J[?ïêt~÷­?hã4º"2t?e‹èiªûV?hã4º"2t?ïÏ¡&"?€Éù·Õ,Œ?x/v¢)ì?€Éù·Õ,Œ?ïHŸ¾C>'?'T£Ëj¯É?–ì7˜-ð?'T£Ëj¯É?ïüö›Â?ChÅÅ9k??`I]¨r?ChÅÅ9kAGN4FGL J0156.3-2420¿¬THÎó:ÀRÈÁæ¯ÍÀ:ž¯ñʳÀ<ßŠ>²Ã@&âéê??ý²øE ›?À"8#²â–?ºÆÏãÉé?ünà¾Y"@
kRË)¸¿ïþ¬B鉜?ïû .y¿Öôý"U"¿åv" 'E¿Õ‹¥|§¿ÝªßÃ^UNASNone3FGL J0156.5-2423?ïÿs┤?|'?ƒ«ñ)?|'?ïô¨'?μ?^¶5þŽ?V¯±ö•´?^¶5þŽ?ïíÑöhÄ?g1!•úd?b.	±C§?g1!•úd?ïÿ$ôè0?	@"v°þ?a]ßÅ E?	@"v°þ?ïþüн‹?dhsD"i? 3Sº©?dhsD"i?ïÔçœmÅ?|۟ÚÙ²?uŒ1«æy¤?|۟ÚÙ²?ïÚ©®±ü?|Û¦'ž3ð?r«(ÁÎï¢?|Û¦'ž3ð?ïýÄ¥G3?(àûâu?1ÚÓµŠ"x?(àûâuAGN4FGL J0158.4+1230¿îÜÊ^'
ÀG"‹—xW*À:Îû­Šè&À<6Îý(µ+@ÔЯZv@9RKý."?ٔ»#6â?éH#à"å'@øÚ¶š[@O°oó?홽 1xÉ¿çd•ÁGÞf¿ïÿÿ" 5•¿ï5A•Ì…?ïÿÿ>¹ú¿ïÿfb4¨~UNASNone?ïÓ¢#«Ö³?ŠÐbÈ;€?v.î—Ʀ?ŠÐbÈ;€?ïÓ¯bŒDÐ?Žàó…dm?v(NÀãÿ?Žàó…dm?í'a­!¿K?¢jlŽ?³tò"ÌD+?¢jlŽ?ïûÁySöD?@Ɲ!sn`?@ú"Ù¼·?@Ɲ!sn`?ï"x"U%æ?òJ³ùq?ŠáÚàg²Œ?òJ³ùq?íž>²?Â/õ±G‹/?³?ŽæVD?Â/õ±G‹/?ë=VW?­«3ZVí?£²?­«3ZVí?ï]ó,õ?™~çSÆ,ž?"Aâù™e?™~çSÆ,žAGN4FGL J0159.0+3313?éÝF"ÑóAÀ;ÎázûÀ;avؤÀ<¢‡~äâm@ YØ&ÈÙ?ÿ'äÓ?ÇiËu´¸?¶eΐò+?ñÏîTÜÑ'@	Ò¯4‹wî?ïíJÖE¿æ¤œ—zÛh¿Õ°¡]ˆF`¿äÁ—½÷¿À¨W{'ò¿ïÿý¡UûŠUNASNone?ïÿ:,n}?ZPUfñ?ºt™»Î?ZPUfñ?ïö(©þ|Ù?Uö"lDQ?S®«—Ò}é?Uö"lDQ?ïñ
q,½ù?aw©o#ž?]å3.a?aw©o#ž?ïþΫ8?›+€[´?/ÓæÌoò?›+€[´?ïÿ1KQ?s:TÅLH?֘m­Õ?s:TÅLH?ïÖÈ£L(?}'v…ó?t›®{	×á?}'v…ó?ïï¨ûc'?mÐÐa\´\?`Wè\ˆ÷?mÐÐa\´\?ïúꕬ?<ÿŽÀH—5?GøXc'Ð=?<ÿŽÀH—5AGN4FGL J0159.8-2234?çXïéÎÇÀRv¢‡~äâÀ;ªðÏ
•À<ëžÈ­ƒ[@ ö=@RU?ö•ÉæhE?à»E¼Cé?ïÌýߔO®@» 'V†õ@9A‡´¿»¿îâáH2Ÿ?ïÁí@	ÛK¿ÔäçßCr?Î$Œç¯|/¿èÁèm<C}¿Úˆ\ÛMC*UNASNone?ïíê•EÞ?gØ"K0?bj‡G±i?gØ"K0?ïäQ^ӆ?r¸¶à:^"?kú®Ç¨•?r¸¶à:^"?ïp(¡ß¹9?†Õꉟq7?'úë½) ö?†Õꉟq7?ï‰G¹ú'?xÛ8ÿ‡«w?®Á`—v?xÛ8ÿ‡«w?ïqèT›?'6PèÞwÛ?'Âì\Ъ?'6PèÞwÛ?ï¤ïq£—…?ÍoC¡?†Ä#š‰ºœ?ÍoC¡?î½ü8Æ?›ƒòØË?¤ >m[ʗ?›ƒòØË?ä5Ò¨?žç훖¢X?¦¤'ÀîXt?žç훖¢XAGN4FGL J0202.4+2943¿ì™b½"À>¨
¿v¢õÀ:æëlËvÀ<Œ<´¼4Ï@ϖ‡å<@áa¡Û‡{?Ä¢J˜)¬ø?xÝmÒ¸c?µ·g	úTÅ?þû€'µÊ}?ëUx™]4¿å#¡Å¸¿àwñsuB¢¿ãÉűO˜Å¿Ø˘"Æ£¾¿Ü­Hãs­LUNASNone?ïý©w÷Í?'¼çQàSÝ?7µvQˆ±?'¼çQàSÝ?ïô¿Æ½'?VŒî¬@ÉG?V€sÔHL6?VŒî¬@ÉG?ïñˆWk»?RdðvËe{?\ïPÂԓ"?RdðvËe{?ïóšYzp?<h(B?XËéµ@	?<h(B?ïútê|yè?;ÜD@ØßF?F,UÉ`0Â?;ÜD@ØßF?ïÒá+~ˆò?}ƒü3JºÎ?vjF:æø?}ƒü3JºÎ?ïô¿Ž1ß?b;ºr*Š…?V€ãÁŽ0×?b;ºr*Š…?ïÇÁÝ?huU9fØ?|9%m|J?huU9fØAGN4FGL J0203.9+8120?ïÏ¥ªÒ"¥@2ݨG²F9À;"Îñj;À<ª<"¸@ §/"R
?üBöõ•C?ÒN{ãüa?ѳôC‰A³?ýT£
[£•@!ٻ̿ëÍÂ6Ƽ?ïÌ$Ñp |¿ã¬Þ²þE¿Ç=:ˆ'
Y¿äôdUêî ¿ïþߤ?åÉUNASNone?ïþYçteO? ˆLeZÒj?*aŠ]®€'? ˆLeZÒj?ïí0d?evH"DÈ?bøý²¾ÈÄ?evH"DÈ?ïãJyú?a€qÀ¼½?lôµÉKö?a€qÀ¼½?ïåxn•x¼?NÆò™Í?j‡'/mûä?NÆò™Í?ïþÃÎæl?´®´ù¢ü?#Þ¨"Ã?´®´ù¢ü?ï®°	G§^?Fï â?"Sý²åœZ?Fï â?ïàåÑ¢í?sÖlêT>;?oæásj?sÖlêT>;?-·É0?x×'äÏ?ˆô£;À?x×'äÏAGN4FGL J0204.7+6656¿Õ,·¿cG@Tâó¾ýÀ9¶ZöƛZÀ;˜í8}@ݪâ`@ؑüí&	?Á °å¹±?Õ›e Á@°Ì¼Õ,?ý0é5_?é²X­@?‹¿Ö\çÙßZ¿äèÈ%ž¿èÚ'Ér¥9¿ïÂ[ßú¦û¿ïþ¼~K	"UNASNone?Ø,´­5?ÈoálõQ?ãé¸%©er?ÈoálõQ?ͯ/-?Åà³g)?è»Ô8ô4½?Åà³g)?ⅎJÏÃ?³ªßä—ôÈ?ÚôãÅj`z?³ªßä—ôÈ?Ô²º×ÈG?¨·¡å•?妢"r›Ü?¨·¡å•?¥~dÉÚß?©DÒíÇ[?î¨yŠ'?©DÒíÇ[?›ÀßW/Ç?¦`8¬±?ï!ùò?¦`8¬±?¼aŸ_ßÂ&?§1•Û;Rü?ìsÌ»?§1•Û;Rü?eõ·®€Ò?t—=G(ö~?ï|ÐR4͊?t—=G(ö~MIXED4FGL J0207.2-1832¿â՚8svÀQ¤Þ*Ã")À;5Ç/ÔÙâÀ<ŒN«^½û@C,[}ª@êB¡e@?ÍSW@Ïh¿wêZ½•ì?§{R[Âsƒ?ónÒHaÔ?êšCb«Eé¿éýöHò¿ßƒ3ü†Î¼¿çŽ"'Ùc´¿ÜÜT^ü噿ïîQ Ü"UNASNone?ïÐz#z?®›EÞ_?wÂð+rÔ?®›EÞ_?ïÛ­ú"sT?ƒù›Za'ë?r)•ú[?ƒù›Za'ë?ï›x%¢ô.?ˆ–J]0?‰!ö¡'È…?ˆ–J]0?ïçAYUu—?R>¿[‡©š?h¾¦§Ê¸ä?R>¿[‡©š?ï÷Cñúâ<?Xnd•‹ü?QxItV¬?Xnd•‹ü?ï‹=
°v?›
Á3˜\?0¼—g¾•?›
Á3˜\?ï_ÎzÝýÞ?')V.˜–P?"0¤@DF?')V.˜–P?ï+ @8¢?‹Pî`ïy¸?š‹÷óÖ¡Ä?‹Pî`ïy¸AGN4FGL J0209.8+2626?ë"Îa<À@›OKD¢À:묊7&À<P{B–~@ÖMô™=@'°Ì¼Õ?Çe¥`ÍX?¥¥
|P™²?Ûe5ŸŸ@†œñû€¿ßDÙ»J¿å$ #!¿æ› ¢ŒÝI¿â}ŠuV¿æcü^ŠÏÒ¿ï×þŽæ¸0UNASNone?ïýz´ÒD?%žË$~Ï1?4*YCâÞª?%žË$~Ï1?ïóؾ·O&?\É4µëê?XNƒca?\É4µëê?ïìî´d\\?ZÃ5Pòc?cKݜ#r?ZÃ5Pòc?ïô÷D*ãj?:3eãúÖ?Vx%ëù?:3eãúÖ?ïü¾>êv?15T''a?:⡅?15T''a?ïÐé€Gõ?{ÙòkÂÎ?w‹?ò²Ý1?{ÙòkÂÎ?ïèïM2ì?p^'Ü?gå~"?p^'Ü?ï½ázay?n_¸·X?€¸©N»Í?n_¸·XAGN4FGL J0211.5+6219?ïª<6'
^?ìXu—5À9vZYê
À;?®ª@ÒÆÛD)@ã.`e›e?Æ$nŸDÿ9?¸½èƒažÖ?íêsÁ˜¼$?þ¾¬Ÿ/Ü?Ôh`;©ú:¿àâíP¿é"@U¿å<jŸ01v¿íEO?ƒM¨¿ïï¶Ü gUNASNone?謹üÚ±'?†KýªFWV?…P»•+œ?†KýªFWV?ï0	] í`?Ÿ‰ƒÕj³±?™þÔZ*…õ?Ÿ‰ƒÕj³±?íßò-{ې?¡'¥æKQw?±n'×I?¡'¥æKQw?î
jfÓ/?'[¢Ã,ó¦?¯)_¶ÿ?'[¢Ã,ó¦?ìupò}ØÀ?¹+UäÑ	ú?¼Txl9þ?¹+UäÑ	ú?èçÀ·¢»?ÌnP}ã?Ì`ÿ!u?ÌnP}ã?êí¼÷AÀj?¯LŸRq5?ÄI"øþY?¯LŸRq5?áÐL‰›?·~/\Yµ?Ýü_fíÊÉ?·~/\YµAGN4FGL J0215.0-5330¿Íš|ÖÈרÀM¸H@áqŸÀ;¤†*QbÀ<ër
—@ 
mý´v?@ßËlÂ?ÂF(XcÄK¿À‰¢«'â?ó]]Äuq@ß&–—²¿éS®2­Ò6¿êµ0-Å5)¿áqô¿Zƒ¿×õ·ý‡Õ¢¿Õãm"BJ'¿ïû¥]:ÉUNASNone?ïýá±z$Î?0vP9¯–'?0òt]'Ï?0vP9¯–'?ïöHÏ&Ä:?TŸÕñ­7¡?SnaéqK±?TŸÕñ­7¡?ïÞDñew?|vÞ̆-e?pú]<@S?|vÞ̆-e?ïþ¼Wþj?ŒIù2¾c?$:Šå~£å?ŒIù2¾c?ïülWl""?5W"W•cï?<B·Õýð?5W"W•cï?ïØR+ñË_?ya™¯j?sÖê?ya™¯j?ïÕbf_?ªE>E±u?uO{|ª?ªE>E±u?ïñ¾È
†?W±†X߄?\'o³x‡5?W±†X߄AGN4FGL J0220.1+1155¿çƒ×&(CýÀF´ê¿üÚ²À;Ñù®­'À<̹kÆøw@#£
VE1
?õS"¬¢ŠÚ?Øléã3¬?Ëv远Ž?ñÌI"®P
?üwŠ*ÍB¿ïSIˆà
ò¿ï웟-WQ?å
ë ¢wd?è7¢cl¶â¿Ç,>¼~K¿Ô''>[…bUNASNone?ïý'KK?/÷R}ò3?6ljý)Ý?/÷R}ò3?ïôO‰!Ÿ?Y'!mG‡ý?WÉ`Ò?âË?Y'!mG‡ý?ï͞™]´'?ySˆYՅ??y0³`óë_?ySˆYՅ??ïû¨þø>?6Ñ½T-?A\ª3¾?6Ñ½T-?ïýßÉv""?*cñÆNÔ?1µÔãD?*cñÆNÔ?ïÐö¯–¨p?7'("CM?w"¨%€?7'("CM?ïÆM±†Ò?ƒft|t\Ù?|Ù'Rò¼?ƒft|t\Ù?ïò/ԝÀ_?[)û²W?[ Vž£?[)û²WAGN4FGL J0222.7+5016?è%H‡Œ.À#þ½LýÕÀ:âÓº&×ÛÀ<}œ¸2@ –Æ*œ6@˜Ð`Ö­?È\[öu菿Ÿ.'Û+¬¤?Öì˜ú¸B|@L+Dý?ï÷ýÖÚî¿è!"hýð¿â"ëSÏ¿ãÿëþ@bF?'o¦ß…ꙿê7]>ÊkUNASNone?ïýüüÚŠ?#*'@$[±?0Oÿì
?#*'@$[±?ïô™R‡R?\ÁW@^5?VÍZâ´Ë?\ÁW@^5?ïõ…Í"ÌÍ?X•[–¶\?Tôe´ç9?X•[–¶\?ïýÏd½Õõ?g÷´ë‹?1"Ú)€Éä?g÷´ë‹?ïüÎFÁÒÀ?3³±]ޕ?9ÇÜ&¡Ê?3³±]ޕ?ïÆׁþê¤?Šrà)«2?|"?W¢?Šrà)«2?ïõgóÚ,Ý?d²`&¾«+?U0˜†;?d²`&¾«+?ïõޝžzÄ?J9µg?5?TBĜŽØ×?J9µg?5AGN4FGL J0224.8+2937¿©Ã–­«õ<À<ÿÜ&Üã›À:¯Úv»œÀ<I½ò>v]@`+ŽÏ@.ȺïT·?DZ%fìÉ?ª;§\6?à‡f%ÎÆ¢@ajþüu?ÀvD?u
ï¿ëŽèe¯‡B¿âsՅ2à¿êcA¹óê¿å•€¸Í¿ðUNASNone?ïý¦t|i?+Ռ•/ÿ=?2ÌZC¶
þ?+Ռ•/ÿ=?ïô‹®'"â?\Ø D?Vè£-É<L?\Ø D?ïæß¿\"?k"QH#¯?i @~S¤¹?k"QH#¯?ïõ¤÷	¦?:ËDáfâr?T¶Aê9Ô?:ËDáfâr?ïý"Öq™Ô?3fœé›"º?3ÙNjÄëD?3fœé›"º?ïÒ´1½!?~+Mâ'+?v¥çD¶?~+Mâ'+?ïÔ¹a¤Ïr?xøµÎK"?u£O{?a?xøµÎK"?ï¸yóý?ph¬˜£9?á˜'Qæ˜?ph¬˜£9AGN4FGL J0225.5-5530¿ÚÞ`Å´÷æÀLvi¾	»kÀ:e'Kí>\À;ÑöÌz—v@‡_/es@°yK!?º!ÿ¯"B¿²ìÈío/?÷t'òÜ+@òÎO§Þ¿èï!áQ>6¿èsшô¿â4¿Ÿè"'¿àJ½ÞYÿäÉGNΚ¿ïøHEéïUNASNone?ïùByÕ·‹?B|Å®	?JöPÎĈ?B|Å®	?ïñÙ/Aó&?`',›Š?\M¢ÊcÕ?`',›Š?ïÁ|ù*g?2aCDJ?Aƒ}*|›?2aCDJ?ïóތ<ä¸?Bq²Ž?XBç;ÿÇ?Bq²Ž?ïØN?uƒ1?oã°	æ½H?sØà'±Ã‡?oã°	æ½H?ïÆä^?ˆ$Q?¤	ÿ?|þýªØ¿?ˆ$Q?¤	ÿ?ïWϸö'T?"Y떬ù?•ÜK€?"Y떬ù?ïd3´ôz!?‰Cy'Ã/£?"y‰ap»Ý?‰Cy'Ã/£AGN4FGL J0226.9+7744¿ç€­Óž‰T@/©	¾ºÀ;f6䘛mÀ<´ÍǞ@!Muþ‰Þ;?þJÃ")´?Ð_|½@?º}=msËÕ?ïÎùͶט@N‹•‰¿ë°ûœÄ?ïÐâ (z?èF4AÑ¿åá3÷~Q?¿ØáDŽ$p¿áò,}a¢UNASNone?ïþÊHÁ˜o?:sQÄO•?#[râüú?:sQÄO•?ïí
d?drõ
ƒï?bæþºx;ò?drõ
ƒï?ï끶µ?]Ew&QÌD?dà~°þ¼?]Ew&QÌD?ïØê?¬ñÄ?]½ô:üŠ"?sŠàFcÖ?]½ô:üŠ"?ïþAjó,Í?$Ìðٍ[?+éT³Ž|«?$Ìðٍ[?ïªæµr?­CBëz?…FR«»³‰?­CBëz?ïã‹úŽjÖ?tölŸ5Èã?ltp5QÛ?tölŸ5Èã?ïŒ'-ôãu?~³õb?Œö4‰¦Z¾?~³õbAGN4FGL J0230.3+1713¿ï)±5±V"ÀCÉ\ú¬ÙèÀ:a"»ë$À<J›ñ@A€§…?š@ðHðŽ?ÈÿQ™Ð¡?șß9¶Úó?ü8­uïpf@QüïÕ:…¿åNµY+¿á†…‰A]¿æ@O±;`¿æAözE@|¿ïÿ"àT¾ô?ê&f%ÎÇUNASNone?ïÛ²ëûW?m î$¼?r&ŠTŒP?m î$¼?ïçøCÀk?o-:ýÓ
?h¼/S4?o-:ýÓ
?ïŒÃ]jòÆ?–ÒŽ˜¤?ŒÏ(žd›?–ÒŽ˜¤?ïÍNT¡ÂÞ?cIúGHÜÅ?yXÕÐ'á?cIúGHÜÅ?ïS¤q'ÏA?•ˆea%+U?•‹qÞu³å?•ˆea%+U?ï>¯ªÔÄ?¤&;Ç?˜*.v?¤&;Ç?ìh€Ä­æÐ?©ÊÙ£7·?¼»ùڐɀ?©ÊÙ£7·?휘َ?£Iõ¤SÔ5?³?U‹?£Iõ¤SÔ5AGN4FGL J0230.4-1140¿ÕNlþ
ÀÀO"[t›À;ãeUÅ.sÀ<åycՒ@"Eñù31?öœªÆÇ©?ݎ½"à¥?ÔÐ&žzT?ù&Ui¾à{@õ•íg¡û¿ï.G P ¿ëÀãàd¯,?ï÷áî-¿ÛW
Ãbó?ʋ)¿A¿â(Ý9+š¸UNASNone?ïý8}Ü
?,ý»?3†>/.ÙG?,ý»?ïõ\ãRA¹?Wæ¨zž;?UF9 4¾N?Wæ¨zž;?ïÏJÀîr9?wn;ê3\p?xZŸ¦u?wn;ê3\p?ïÿŸ?föêŒ?<vcZ?föêŒ?ïý´ ân?3ŠÜèà?2^ù®3¹±?3ŠÜèà?ïÔ9ä¹cË?}g-˒'œ?uã
°\ž¥?}g-˒'œ?ïÚçÖ#Ê?{Œên$I?rùŒ*;¯?{Œên$I?ïýEÿ¤Ì?6êï¼C1°?5ÐÙ<2Ù?6êï¼C1°AGN4FGL J0231.0+3505?ìAdi¿"ÞÀ7wÂôÀ;¥`úÛ4À<ÓW,6¿°@!õ¸¢žP
?ÝáÓD59?æ¿qdÇ)ö?ïÿ¯Èe_@SÞ|!¹Ž@‰\N4–`?î`pî¤ü¿ì¶´ÝlØ¿êނ׶4Û?䗖ºÖ*¿Ô:睸0¿è'#ᆘ5UNASNone?ï熞·ˆ?nE*Ã)`N?hyaG‰?nE*Ã)`N?ïðn¦ë€†?eÿYG+?_"²†tS²?eÿYG+?ï,{¢Òl?•¯–`H!ÿ?Ÿ:pNt?•¯–`H!ÿ?ïë"*®n,?Z(Ě}µ?dlՁ¬[÷?Z(Ě}µ?ïÝkõÛ^?{á;œòt?qJdõIW?{á;œòt?ïÂÚî×Z?‰®JWqhé?~'ˆv8Bö?‰®JWqhé?ï+›H螇?–a?fñq_?šŒ–Ü÷-?–a?fñq_?ïܺ,ÙtG?vD·áIƒÇ?q¢éxxèl?vD·áIƒÇAGN4FGL J0235.3+5650?ÄPw¥¼
À	ŽØ'ãt¯À9­Ž»ð·À;§³Æk‰¼@Š^nJ`v@Ð >cé?Àã[š£~?×êÁªYÛ>@¦Ñµ(k@KªûìŸü¿ÓÌŸóOî¿ÀùÖZÀ¿çA>U¦%¿êœ}ÿà¿ìèÓ=ª/"¿ïÿæÀ
UNASNone3FGL J0235.7+5647?ãj"û>%?Èv0=µm5?Ù*Ö	ƒÙ¶?Èv0=µm5?æå­Jó»›?Ê5ó¢#«×?Ò4¥jˆÉ?Ê5ó¢#«×?çÏ[¾¨Øã?¯œ£-Nê4?ÐaH'®N:?¯œ£-Nê4?êªå}g?šýÐ˖?ÅTkãº
d?šýÐ˖?ƄÝ'†š?Á¹žÐB֝?ê^܈›^Z?Á¹žÐB֝?ÂRç›&®ã?Ž¬Nä$é?ëkF6TG?Ž¬Nä$é?ЖÒgÉñY?´{YžÌ?紖ÌT?´{YžÌ?Ì*‡y?©uZ+6èß?èõ^:a¿|?©uZ+6èßMIXED4FGL J0237.8+5238?êyHL¹°ÕÀ®–ÃüC³À9ÅÛ_6Ç<À<VÁ1Ž…@Vá:B.?üèM&#€8?¾ÎG*`ý?㎧Þ*î@ tNrSÚs@T	|€"¿©q¬]f–¿Î÷çؖڿˮ)7'¿ã®T§!A™¿ïÓ4*…¿ïÛgNnUNASNone3FGL J0238.0+5237?¡z«ñú"?µý×÷AMO?îèU@›ø?µý×÷AMO?Á7†T~™?¾ÚeÍË`¢?ë²9jàZ?¾ÚeÍË`¢?²Uè>ïß?¢_# T?íµ^c/Ä?¢_# T?³P,¥:ç¦?–ñ•Ãœ?í•úktë?–ñ•Ãœ?—…K…™ÅT?½¾'CÜE2?ïCÕ£œ8?½¾'CÜE2?Ÿ÷+í…S?§DÇ«8?ïF ½5?§DÇ«8??–\½	$?wFÜ6çè›?HS¬?wFÜ6çè›?l®‹xðˆ?\±ÉD漞?ïãQð§aG?\±ÉD漞PSR4FGL J0238.1-2621¿ìՏÂ2ó{ÀPŒ¢3œ¿À;쪸¥ÎÀ<°䭔"@"³Ä=1@"Ã9¦?ċšþôg¿Š·t˜O¹ô?Ãþ$@­š@
93Ù?ڋւ®°¿ê3*š}£¿ã›¸øÚqÑ¿ç¼àáVǍ¿ãÁ2d×.¿ìÚ¡oBUNASNone?ïÿn
Û·]?ï€ÊÑñ.?>Ÿþ­k?ï€ÊÑñ.?ïöòþ®?T70B?RêI8óÜ?T70B?ïôJþ^Î?V'ÜÂâ]ñ?WjøŒÔô?V'ÜÂâ]ñ?ïÿUƹ•ì?3ôül'Q?G0'-DP?3ôül'Q?ïÿ YÚÅg?v" ¬IË?é™î3Î?v" ¬IË?ïڞd.¨µ?xt™tT?r°ÍôZQ{?xt™tT?ïòPF\•?`÷ì-Ðu?[_síˆe1?`÷ì-Ðu?ïýQÖô?)kðɼe?5w†ù5$W?)kðɼeAGN4FGL J0239.1+6634?Ă9ô¡Ð@¦¨¸ñM¶À:!¦+xSÏÀ;¦åßÃI–@K|¯Óí¨@îOá¿£?ËV¢ùê'0?Ì2#(N'Ö@¢]<ñøÖ?ñ
4EHß¿ïþ] o!?ïþ¿Þ§À¤¿çËxÎø¿ã#9 µ—§¿ì¼¦¿Fý@¿ïï–áXuUNASNone?ï@rЛÓ?¡«0'_'Ë?Wñ¥ì…œ?¡«0'_'Ë?㼀—r«w?ÌnV°÷ë?؆þÑ©?ÌnV°÷ë?íŸ)øI\? ã¥i-w?³°>éÎ$? ã¥i-w?æñ½É
Ï?¬qØ]ÅE)?Ò"mëôc?¬qØ]ÅE)?êHýû÷e?Á+º<–"0?Æߤ"k?Á+º<–"0?Â7Üvt7?È5.¤ÇäÊ?ë{²âbò?È5.¤ÇäÊ?äç_u¹ô?¹¬àâó«?Ö1AŒë?¹¬àâó«?Á¬1õyþ?®/ÎÓ ô£?ë"ó'¡¹?®/ÎÓ ô£MIXED4FGL J0240.2-0248?ÈùMØ¿¹ÀK1ÿ`Ï‰À:Ïú÷''ýÀ<{q°F"I@ýw:Ê@g&Š®D?¦‡h¿‡¿‡*[?¹ ?Ã@ŸØMœ@òïÌ+<?ãº4¿O`»¿ê{ù?ò^W¿çAÿI ÛB¿ç1‡+ØË߿ҟhûìõâ¿ïþú·ŠñUNASNone3FGL J0240.0-0253?ïþø»_‰u?q¼ ùöG? tKxØJ=?q¼ ùöG?ïöHÊÛA@?U¿çC>×?SnjI}€?U¿çC>×?ïôIaP†?SÞ?ÁWû?WÛmÁOô;?SÞ?ÁWû?ïþýŸ[-+?
V#8!Í
? &é®ì?
V#8!Í
?ïÿ>Î`ºo?gÛöð¢?&-f·E?gÛöð¢?ïÖ·À(Ø?{º¯ »ø™?t¤ËGŸ¥?{º¯ »ø™?ïñåå;ra?_'=4ªàË?\45†[Ž›?_'=4ªàË?ïú¶3Љg?:%ÿú]G?E'0Ý0ls?:%ÿú]GAGN4FGL J0245.0+4755¿ì(;þˆÜˆÀ%vbwÄ\¼À;õ5¾À<X;ãv@1ˆc;d@+­Ûoý¿?Ƈ%£¨'.¿˜Q§E1k?ËƟ¡›p´@ˆH®ðn¿ð?ïÿÿ^ðP`¿åMv«Xÿ¿é'öè)J¿Û­"\›Œ¿á2ÚþhÑ%UNASNone3FGL J0244.4+4745?ïý¼;㎎?3Ôo‹Œn?2!Òýà?3Ôo‹Œn?ïô·&Ùo?\æ {¤u?WȑµÒL?\æ {¤u?ïyÅҘÏÖ?:ƒIüt?ÇE©vi:?:ƒIüt?ïüè¿áF?(ÎеOåq??ˆ¹ÂI¿?(ÎеOåq?ïü)•5íß?<Ñ"ÚÎ\?>³Vîånÿ?<Ñ"ÚÎ\?ïÁOÆf×%?‹€Ùyñm?XÝÂyž?‹€Ùyñm?ï~?h ¨W?àéï…O?8å½5?àéï…O?ïå«ÇÞ?U?`Þ7!ºô?jT8bYRã?`Þ7!ºôAGN4FGL J0246.0-4838?ãåêmFª^ÀM£~õ©eÀ;(×å.ÃbÀ<h¨-±@ç×õÊÇå@µî;²]¶?Äç©Ý^•b¿ºHY`™?òI²Çh	@ˆú:U¿çO¶@ï3¿éG¿å‹<¨&û¿åJæþ§:l¿ïÿýF\I?ïÑ6‰)	UNASNone?ïõãÀóêb?S½=ÂìÞ?T8~¡››§?S½=ÂìÞ?ïñ}|"µ?hõRR_TÄ?]ŽŸ]?hõRR_TÄ?ﴊ‰w¹?‰42è=?'Ý]·jãÂ?‰42è=?ïü8更ï?0÷¦¸Ž˜ß?>8"gÇ£?0÷¦¸Ž˜ß?ïñŸÿS ¨?b"Äú"(?\ÀæKÐ@?b"Äú"(?ﲸž}Ý?'8NÈ\r?ƒQØu±ŒÇ?'8NÈ\r?ï¶c}?…†	ÐÖu,?'|Üœxê?…†	ÐÖu,?ï¬/>Ã?€‹m•}Ø?"ô0Dê‹g?€‹m•}ØAGN4FGL J0251.1-1830?åcy­H«žÀN—ñ{ؾsÀ:öbWãì¤À<pD5¹ö0@!vfóT ?ôç"øoé?Ñ8՟eæ?Ü_õ~F×Ö@Ò¯dÜùk@7µ	Œ›¯?ï0ÒÐòÌ;¿î×Û'Ùc?éätSŽóM?•Q:]³¿Ñƒ˜{au;¿ãáý`"iUNASNone3FGL J0251.1-1829?ïléGÉÄ?'VM9z½9?'b×
Ÿ]?'VM9z½9?ïà`k-S(?"òF@ú?oŸ"Ïí(?"òF@ú?îGzDŒt?ž;'»pSÜ?«ˆ[¶b'À?ž;'»pSÜ?ïÁŒ·ÞÔ?p÷ûœ?9£ðù'?p÷ûœ?ïÍQ¤YÞ?Œ6Ú¦Œî§?Œ«"yìk?Œ6Ú¦Œî§?ïmÍCÑLJ?©€7Œ£?'FW€¯Ô?©€7Œ£?í;ª9
Hê?§uln·D…?¶"®8‰Ÿ¬?§uln·D…?ïLúZ­(?":rR†?–|À¬U?":rR†AGN4FGL J0251.6+0628?Áÿ\þGÀFÉD€bïÀ: ­‹¾åƒÀ<'¤ˆ
%@2au»Ä@ZYÀe¶=?ÄûZiXU?¨«œÀ.rž?á—ÈAíá@ópOžN¿ïn'>´Ï?ì'VÃ[4¿í?Í«Þ¿Ú4çhY…­¿ì_Ïsp:?ѝV}JKUNASNone?ïïBÃt?‡?üÒöré?`½<º²M?‡?üÒöré?ïóEÓ¯ü?`kÏMÜà?YtXqM ¢?`kÏMÜà?ïyªÈ¸b?ˆÜz&Ó!§?Ê¦å"&?ˆÜz&Ó!§?ïö²Ã{E?<ÁÀ&×	Ì?RšxÒÿµ»?<ÁÀ&×	Ì?ï¨9\9‰0?‹šnïË?…ñ¨ãßD?‹šnïË?ïÁçvFXT?‡ºRoæ!E?Dç"©ò?‡ºRoæ!E?îô]·—Ð?˜¡ÈO*-Ó? º$ˆÞPý?˜¡ÈO*-Ó?ï¬0W-0?yìlÜ>ˆ;?"ý3Ù¨!?yìlÜ>ˆ;AGN4FGL J0252.0-3657¿ï!ÁÞÝ£ÀO`˜²é̸À;ŒôNÀ<꬇²çH@ :¬þT?÷ó朁«f?áHÌ!¬"?ÒMÝC¢•?ò+Z;µ¸´@jOøË¿ïüùOâ–c?ïÈNòÄ®¿èEr/ÈD¨?'{o"i©¿æ~râÅB¿ïëá/Z`ŸUNASNone?ïþõÿÊ?T'ù±¶
? ®Ü'5°º?T'ù±¶
?ïö°zlê?TsõPx?RzŸ~™Í?TsõPx?ïࢉq?l3ň—Š?oè]—úÎä?l3ň—Š?ïþ—q\?Ù&Ê à?.îG=<?Ù&Ê à?ïÿ·a;ëO?…y®ü™i?'Ác¡¹Y?…y®ü™i?ïÙº¸ðn_?yu@³L?s"£ÆPd?yu@³L?ï၉FT?s˜33zS?n~vèfž¬?s˜33zS?ïû¶o=O—?9ìˆA4Mg?A&B$h£?9ìˆA4MgAGN4FGL J0252.3-2707?ï÷72W|OÀO•[0HÀ:Þ\î 0À<¤¯¸k@…kûü4@x¦f0·?ļÚçB¿¨DŸ[f?Û$[)'=@æ"B€¿Ãø*ÞûÎm¿êWådsG¿ëˆ{¯£Ç¿ãýBJþ+¿àvžÝ¦8ä¿ïÿÒkÀUNASNone?ïÿ
̄?%Ó]0ήö?¦kÜ#ì?%Ó]0ήö?ïö9®³˜Z?[«'¤Õÿ?SŒ¢N—½I?[«'¤Õÿ?ïÞtžÈú?rÊ#M*¶Ó?pÅ°ó+G?rÊ#M*¶Ó?ïÿF™cá?9§°çLø?,ÒAFž?9§°çLø?ïþÒŒâ?,j7vüÆ?"ÞøMT?,j7vüÆ?ïØB{‹g?y…Úì;zD?sÞŠ(o?y…Úì;zD?ïÝI<'‹?v¢ÿ7ð=?q[a½™¯è?v¢ÿ7ð=?ïøöYõ%?D­ˆ(ñª?L&—-û©c?D­ˆ(ñªAGN4FGL J0256.2-0408?ÀS¬dÀJ2ýX…ÓÀ;Wy{ ÔÀ<²°9ï@ »Ûۈ?ÿª÷	º?Ó÷e<DÔÆ?¯i³í'Ð?܆p|¿Ä&@GBW=?ïضDË,¿æ
¨ÐnB¿ålKîñ¿Ôè™Fƒ¿ÞZZT	l¿î.R¬,ÄUNASNone?ïÿˆÆã~À?ºðÿ?
ÎC82^?ºðÿ?ïö¤§i»Û?T•9?–2Ò?R¶±ŠÉY?T•9?–2Ò?ïù
y¾?ZI]¬¯|)?KÊ•P̈́?ZI]¬¯|)?ïþt}^G?'%ó·(?(¸-Ó¢ø?'%ó·(?ïÿÚéù‹û>ëð†?Ö{2>ò‹ý\›>ëð†?Ö{2?ïÙT!ÀD(?x­‰ 1Ç ?sUï1÷Á?x­‰ 1Ç ?ïûM­vµ?Q
P®ïÆ:?BÉIÚg«à?Q
P®ïÆ:?ïû63ëa?6KK	Üm²?C'¨;€åó?6KK	Üm²AGN4FGL J0257.8+7044?ܶ–f֛$@$ËYWŠ*'À:6ÄÂ<PÀ;Áœ¸2@»	sq@N`›KJ?Ä̎c…‹p?°ˆ›ÅmÝÔ?ç?	ËZÜÅ@~Ñ{]A?ïï;At"|¿ár%acr@¿æ,æ³'à¿è¬ôŸú†Ä¿çrSÚr§½¿â€fWLíïUNASNone?ïøà©­R?CL[5?L'ögØ?CL[5?ïØÕaÏ[{?v£3>ý\?s•O'pŠi?v£3>ý\?ïÀRVÀ"?xoïÑZW?ÖÔþ>Á?xoïÑZW?ïÓ4l;?jP–í)%?‹Ë:yÄ)J?jP–í)%?ïÞ&' Ç¥?jÈvw½¾?pììI•?jÈvw½¾?ï
"Ó>¬?¤b4'ÿÄ?Ÿ~[£à\†?¤b4'ÿÄ?îÏ®ÆÁ4?˜apC›?£UKºÀ?˜apC›?ì}.ñHñÐ? Z­V­U?¼ˆu¸q? Z­V­UAGN4FGL J0259.0+0552?ÜàvG"ùÏÀFiÕ^kÆ"À9Ìü}"€UÀ;êêÏS)@˜{RÜ8?ýì}6Œ"?º–R<bÜÄ?ÁÔDe_«6@Xî¼
ݪ@	(±‡w@¿ï¶öÁèÃ"?ëX½0w—¿Ý{>ÊÁ¿ØV«ùµä¿ä÷9½ï§¿ì×B4ÍgUNASNone3FGL J0258.9+0552?ïþy§®&¼?" à9^ÍË?(e‡ùژÂ?" à9^ÍË?ïòèJÆg?_9
™ñÛ1?[î/dóÒÒ?_9
™ñÛ1?ïßvÂÃ?tè'ù±b?pDŸÛÖ9?tè'ù±b?ïãáéèo?P›cZ"¼+?lÿQ0ؑ?P›cZ"¼+?ïùÓí—6'?E¨ÁFlÁž?H°H—÷Î?E¨ÁFlÁž?ïËcY8"?~¯ÚžÕ—C?z~NBåÏ?~¯ÚžÕ—C?ï•M²:zO?‹û¤àüWõ?Š¬"mñÐ0?‹û¤àüWõ?ï…Ý…_X‰?~»%äúÄ?Žˆž¡J¥Ü?~»%äúÄAGN4FGL J0300.0-5908?è2}(ØÀIˆõn¬†À;¶,c5Y~À=™'óe@ 8ÅßÉ?÷Ũ›•\?ãp"'0Fo?ÛÀ?øzDàÑ@hÀà?áÒ¹Ág‰¿çâ,Rƒ[¿âü»§á[¿Ì!ðj¶­&¿àÏà}ƒ¹^¿ïÿ‡4<G¯UNASNone?ïúy,́?B©GsìŠõ?F¯opsô?B©GsìŠõ?ïöLéÎÌh?TaŒ‰Û?Sf,² ?TaŒ‰Û?︙DgÁŽ?a˜ D3"?Ù®åºŠ?a˜ D3"?ïúV¤Á.Î?0df_¨?F¥m´L(?0df_¨?ïüoÓ*<?=Á1>¸‹Æ?<hWçý?=Á1>¸‹Æ?ïÙD,)Ԑ?{ג§a?s]éüCÄ?{ג§a?ïв›PÜ?€§Z~O?wÀ&®8	Î?€§Z~O?ïð$ñ"š¸?S"÷»Ý?"?_¶¤Sñj?S"÷»Ý?"AGN4FGL J0300.4+3450?ïԌKt¿èÀ4ìûTŸ"…À:Þ½Ÿ¤vÀ<X®^L¼@pâ²gEß@—XA	µ‹?Ѻˆ¼ývä?Ïg¼&âAÿ?ö	Ã}˜²@…¼:…@?ïæ|Öë3À¿æeÔp/=¿Þ*t]J¿é\#ý`='¿ïÿü¥¬¨?ïH±(UNASNone?ï߅`ƒ9?n'ÛSpH?p=Où]ë–?n'ÛSpH?ïãUԌ£?tƒãZõóK?lª+¨öfù?tƒãZõóK?î惿èÉ?'©ëÕ0?¡—Ä
Øt?'©ëÕ0?ï"Ã$Ç#"?qœ˜Ñlt•?ŠÏ6ße*Ò?qœ˜Ñlt•?ï®Æ ýâ?‡5rH^øæ?"NWÍV•z?‡5rH^øæ?ïGb´3?¡ñÚy7î<?—ß΂¬?¡ñÚy7î<?큵Ør%?¢cIhŽ:¿?³òQ;$üá?¢cIhŽ:¿?ì‰.)´}?¥")?»¶Ž²_ä?¥")AGN4FGL J0301.6-5617¿ïà
½PáxÀJZæ[ê¢À;ŒAÀ<ÐRì6 @ 4±âe»F?û˜ç<º›r?ȗ…4²º?ÊU»Gi@½&fœL@ŸØRg?éÏYoØ¿èBã_5o£¿ÑÈ¡jÉM¿ä9[€Ú0
?£¢y^ˆ	¿ïÿÿÊPËUNASNone?ïý·6Cg?-:B|71?2FM:"?-:B|71?ï÷ ©?S+Ö°÷?Qó؅Ý6?S+Ö°÷?ï×µjtVÙ?tGÌ˴Ĥ?t%JÚr;'?tGÌ˴Ĥ?ïýû¹o,?X}¤'úà?0"7C€`Í?X}¤'úà?ïý!ыùH?5Æp%_M?6ñsÚ{ì|?5Æp%_M?ïÚ®§Mâ?yùžd¡²?r¨¬^{·
?yùžd¡²?ïº3µŒ?ƒ,~°X§?sƒO?ƒ,~°X§?ïøO¶?D#ÀÿÀ^?M¿ÃWz?D#ÀÿÀ^AGN4FGL J0302.5+3354?á½ñ×bÀ5…aܓêÀ;!?8$4À<çÈі@!î>tÎ?ýìEz]"?Ë
¯–:|?˜P|Å"‰m?Ðå³£†Œ@9°â‹{?é ð‹C¿ïÔJ«þ?í]@þ"b¿Ý¨áá¿ÝÂ)ÜÓ¿ÔñÌËö
8UNASNone?ïÿ–‹J¡>ÿ'™úG†7?
d£ß>ÿ'™úG†7?ïöŸÖ8u+?TAÂþûÈ?RÀTÆXÇ?TAÂþûÈ?ïú•¬híï?2ðíH	?E©OSf?2ðíH	?ïøêî²?9Ô3¼oӊ?LTD—LdW?9Ô3¼oӊ?ïÿ¿Àõ©>ô˜ß…)šÞ?·¯÷>ô˜ß…)šÞ?ïÙÔáÝïÏ?| |ì̆Ö?s	XÀ?| |ì̆Ö?ïü³ÒªÝ9?Fj×6à?:aj¼àÆ?Fj×6à?ïóT󙷙?P`Ê¨3?YVÔÏÝô?P`Ê¨3AGN4FGL J0302.7+5717¿Åø–$οòÅ
 ÒrÿÀ9¦é#D¨¦À;@«‡ça@'î
_)†@Gá%Ie¥?Æb Â2À?±Ô9}¥Z?çˆÜä.?ýE´ÒÛÇ?îïsàøRâ¿Ø\&$p¿è¾ne8¿é 6Ff—¿ïç"=ç¿ïÿÚÁ,/´UNASNone?ïà೒Ô?l'Vñ‰³³?oLœžÛE?l'Vñ‰³³?ïlø4ë«?™è#þ'†Ù?'|Àõòîœ?™è#þ'†Ù?îrŒƒ LÖ?˜[3:;¦y?¨×7Æס?˜[3:;¦y?îâ¯ÑÙ?ŒuRá{ý?§áÔÿrÒ¶?ŒuRá{ý?ï•WWL9Œ?>"6ô¡?Šª*3ÐÔÿ?>"6ô¡?ëæe´²=?ÂêŸGÐÆy?Àfi-7"?ÂêŸGÐÆy?ìHø²·Uu?¨'½pN̶?½¸:jETY?¨'½pN̶?åHžBîñ?´{´ç¼?ÕnÃÁz"?´{´ç¼AGN4FGL J0304.6+6554¿äh=*Ì(@Ü ~$É
À;CY7©ºyÀ<Ç
GžÑ@Üv¸îô?þc\ƪt?Ô|_p#?èç~>tYï@
‹(Øf^@Ê.¸Ð¿ïüÿÐ/WÜ?ïtÿ†]?Û‡!F÷‹¿àÓöAC/¿í«ŽÄS‡¿ïò 
¼%UNASNone?îÞ!‡JrÑ?¡þÐҁG?¢çŠ|ëð?¡þÐҁG?é"=ïF@Î?ÇA—3&·¿?ɯBæüÆ?ÇA—3&·¿?íyáä4??Ÿ~¦	{?´0ðÚ¨jˆ?Ÿ~¦	{?æaŒÿF5ˆ?®_ÉÀ—?Ó<æs"ð?®_ÉÀ—?êöÒYԈ?¾­ìPºqo?Ǭ$¶˜­á?¾­ìPºqo?ÝT˙pÿÇ?Ò~'D›îç?áUš3G€?Ò~'D›îç?ç@ĵjõ0?·®[…}Q?Ñ~v•* ?·®[…}Q?Õ<ã*‡=!?º÷â,ãì?åaŽj¼ap?º÷â,ãìMIXED4FGL J0308.9-4702?ßEÉWKìÀLDõýG¾ÛÀ<U¾š#À=,jËOõ@"ókò¬?³‰–íï0?ì(ót'Ý?ïÿo¾ÁÇ@FÍ)Á@,xËëÚ¿ïûÁa´¥å?éßð•ÿ±?ï--àôË¿ÚJ
Dý`?Þæ3:¿ïo¿ïÿñò÷UNASNone?ïůá?¾ÒaƒŸÿ‡?Ÿ‡_Ë»¬s?¾ÒaƒŸÿ‡?ï÷-‡]èû?S‰F'[?Q¤ðÖ:‹v?S‰F'[?î6¸™.l?¡š†š©?¬"vq°Î=?¡š†š©?ïÿDùÚ!?_î{;¦?`ÌËlv%?_î{;¦?ïå'çGæ?|i2²Ó|?jØÉe:H?|i2²Ó|?ïÛS\bE^?x³dg¦áå?rVQڋüÌ?x³dg¦áå?îæ­m$àN?›H!q$?¡•)*B_%?›H!q$?ïÿ¡"ÿoÑ?i;»Á?šÂ"–$?i;»ÁAGN4FGL J0309.9-6941¿Ä2¤ÀǹpÀE}Þ?»×²À;S'¢xæÀ<ºôúé?Ê@u~5ºø?øÎrýMž?Ûh«î/ô?îº@ãÉ@Û¼¾aÐ?øì–ց?ï£^>y¸S¿éŒþ–Ž¿ØWæ'öÀ¿éÍΟµ½g¿ï`Ÿ¨žð¿îs´ÈUNASNone?ïö.2ËâË?^Æãꣴê?S£šh:jÏ?^Æãꣴê?ïp¨>µ??Ÿ¾÷Ij[?'êþùá&"?Ÿ¾÷Ij[?îfž=©j?–SàyhPë?©–!ùÃß?–SàyhPë?í™óž?=$?Ÿ#Ê4—u?³0cNHâ?Ÿ#Ê4—u?ïϬ횉?€"—(€õ¯?xz) wp?€"—(€õ¯?ìÍg:]N?ā˜2³¨Ü?¹"Æ.Ï«Œ?ā˜2³¨Ü?íÛø
þ? Rô&™?± ?‡Á? Rô&™?锝vHÓ?º)`îÏ£c?É­Š&ßè³?º)`îÏ£cAGN4FGL J0311.3+2940?ÝL^Ò73¸À8}E¥ü~À:"å~tz%À<EuU³@Ê®ž8¾@µ¼D¿L²?Ò³A Ùß?â-Ánʸö@	m‰‹.œË@´0©kۿك#€¸¢¿à(ýOK˜¿é3eÞPÞ¿íšÿZc¿ïø`ˆ"?îÜÔ·|ÙoUNASNone?ïÐ0´Ó±Ã?Ë€cÁ=?w祖'R?Ë€cÁ=?ï¬áŽ¿?©—'éÙìÔ?Ÿ*cÇHÖ?©—'éÙìÔ?î°F=ôN¾?""ÎÞ²ÃÛ?¤ûœ"râ?""ÎÞ²ÃÛ?î¡D')?|ASŽF?¥ë½Œiº—?|ASŽF?îÕãs¤´Í?­\kÇÁxš?¢¡ÈÉ$O)?­\kÇÁxš?ã	š°àL?ÓuÙ!âö?ÙìËҞ?h?ÓuÙ!âö?èaT–…=?µÂlí+L?Îz­¥ë§?µÂlí+L?ÚÙÙënM'?À¹åZsz1?â"
HÙ8?À¹åZsz1MIXED4FGL J0312.7+2012?åå¡ÒD¨À?"›«–òÀ:ý=1¹¶pÀ<xŠ§ŽNã@!²ŒÙÔ?û/ä^¹É»?ϞîؐOn?Ä&܍µ
?øI¢@1Hw@o˜Njò?Ûª%?éÌ"C>C¿àMLïœÛm¿¨c¦¬D¿æ¤ ù¿×¾ ºKUNASNone3FGL J0312.7+2011?ïÿ&c
Õ?j"…g§c?3 xlÑê?j"…g§c?ïõ´âö.ñ?U׋?UTÂ?T–9ò¥Þ{?U׋?UTÂ?ïòEvpŽw?\8Àÿϯ†?[uð(aÀ?\8Àÿϯ†?ïöMÛïÄ7?:ùŠ>㍪?SdH3µa?:ùŠ>㍪?ïÿ'WTG!?9C§§êà?ãúb,?9C§§êà?ï×ríw+?|{ËDK.?tuƔóa?|{ËDK.?ïîi³´A?h øsDÌ]?a–Lj4NÙ?h øsDÌ]?ïåúFÇ\?]Ù:~Œ?jr«z3ü?]Ù:~ŒAGN4FGL J0313.6-7508¿î踱jyNÀCd0 ±»ÏÀ:Äs'ÈÀ<n
Jk^@W)ªs[—@©L_T#n?Èôc>¾¬¤?…sÐ -5Ý?¸ñ›8U1
?úoÒ@):â¿æLœ[ùŒ¿æçeÕFîÒ¿ë"–Þ(i׿ê+ÿ,›i}¿ïÿå"m/®?ïný
Ý8UUNASNone?ïý·Aäë–?3¼ºÏéƒ??2Eï6Òϙ?3¼ºÏéƒ??ïÞË÷S¢Ù?…7;†Þ?pš^m£c?…7;†Þ?a19?'Œe'©{¯?Š™'ÃcMŸ?'Œe'©{¯?ïõ¢–ÃPw?Gs¸&÷ò?TºÒú`Õ?Gs¸&÷ò?ïü¡ŠÃ¹?CýàÜÐ]?:ó§ÐáÌ?CýàÜÐ]?ï,]0p?¯ø#
ÇL?š´Yþ?¯ø#
ÇL?ïŒ$Bm#?‰ozbüâ?Œöïl&GQ?‰ozbüâ?ï#ö´t2Ï?"ÂU®ûÔ?›)jšn$?"ÂU®ûÔAGN4FGL J0314.1+2827?ï$*·8¼À8ºH×à&FÀ:•…ú€d>À<³ûD¯\@éeSi´@_yŸÿh?Ë/¥õrˆ^?À¬°Í'Åj?õ?|Ì@Sp?íf'•ù?ÉYF˜?ÒS¿ìr9}û•¿ÙUkÙ3¿áa?èÅQ¿ïýç¡åBUNASNone?ï÷ñÐߣa?MÅc…"[·?P]ï\ì?MÅc…"[·?ïã¤,ùÿ?u
¬¸®w?l[Òûñ@µ?u
¬¸®w?ï±:pÐ]â?ÀÃúu7t?ƒ±cÀ9ۊ?ÀÃúu7t?ïËÌb!eß?`A´+»$?zÎÓ D·?`A´+»$?ïÉ¡nÐZ?'jNÓ¤¹¨?{/HˆÖ?'jNÓ¤¹¨?ï€ÊÙé§	?—´"
Ø>?ÍIth1Ã?—´"
Ø>?îBEÓÚï6?£~im^á?«Û¢¿½Wª?£~im^á?î"£º?›Mà'-lþ?¯µÐ¼-‰?›Mà'-lþAGN4FGL J0314.1+5033?î"dƒÍaÀ—
€Œ'ZÀ:$²øæ0KÀ;È5"_õ@c«¡@¯X}o—h?Íé>]ˆÇ?ÓÒT`ªdÃ@ÉÅ!Ý @¥9Œ=»w?ÔZÙa?ïꧾ d9¿çZ"zy¿äà'÷–¤ó¿ð?ïÿR[§UNASNone?嵐4+Å?Œ!a¡\?†×¿@³~'?Œ!a¡\?ï§>'úؓ?'Wú¬Ç?†0["¹wU?'Wú¬Ç?î	‰|êÀ?œzÌ­uÍ?¯goÇUm?œzÌ­uÍ?ïH1]	4?}#ܘµí?–ùÝû>m?}#ܘµí?îÚ5ëŸK?¤žq`8§?¢^<¢ýÙP?¤žq`8§?ë{ÒÙ×!d?ÆÒ$–s…š?´˜£zn?ÆÒ$–s…š?çÃR^Þ?´";* ?ÐÞy[ûBE?´";* ?éÙj0-Ê?²TûԄ&?ȚW=ÃHÙ?²TûԄ&	AGN4FGL J0314.4-4805¿ßúm˜ÀK¡cÃ÷bÀ;NüÕ©À<èŠF?@çÖA•¡'@ ê@{S?ˁ.(\j?¶Â\ÜNõÜ?ë²_~ØÕ@–É—
MF¿êm§¾Šà¿Ç­¹v®³¿äömŸë˜?¿ÜÂ=|¸7¿åÿ‰b"ʨ¿ïÿýF\IUNASNone?ïþF7O€$?ï펠®?+œŒ°g?ï펠®?ïô‡þÞå ?\ ¯ä 1?Vðâ±C?\ ¯ä 1?ïëIù¹{?]ö%4º?d¶q׋Õ$?]ö%4º?ïø.ª.߉?3ÄcX/í?OEX7ÔÎ?3ÄcX/í?ïþ‰YŸGr?!³,¿Io?'jbbÀ-N?!³,¿Io?ïѓh}?øù­‰1?w6K©g;$?øù­‰1?ïçpÎ/‰—?pôҁ—ò?h1¥ÛA"?pôҁ—ò?ï֝Rƒ'	?e\I*	¨?t±Vºüߝ?e\I*	¨AGN4FGL J0318.8+2848?ã$Ê×^À7×UÿæՍÀ;)-c™ÑÀ<¿¹üæp@)Ç`|B@Á#>?Ù	E#¿¹?ïáµA•Ì…@ë¬c ¹I?ÿ'ž=BU»¿ãLYàF&U¿áãùÚLQ¿¯üòü®´*¿éíô?,­¿ïÿ\ è,û¿Ëƒ–¸h¼­UNASNone?ëC¿¶…†?À˜ßä›dd?Âñ'¥éè?À˜ßä›dd?ésn©yÈ?Å70ФÀ?Ê2GZá?Å70ФÀ?ê5†ÓªrÁ?¬¡tJÓÙt?Ç)ä±V4ü?¬¡tJÓÙt?âˆ×(Š&¤?´¹ý‡»¢?ÚîQ®ë²¸?´¹ý‡»¢?ày(§Wâ?Ϭ:
ËxB?ß
®±P;ú?Ϭ:
ËxB?Ð`ð¥ïé2?ÎA?ó[¤?çχ­g?ÎA?ó[¤?Øl}ǁ~?½õ™¤¬?ãÉÁ?{Á?½õ™¤¬?µŸòj"i?¢‡i{¥°?íL²vy?¢‡i{¥°	MIXED4FGL J0327.6+2620¿Û O	—GIÀ8¦°úß.ÏÀ;E'ømd‡À<—ªÉlÆ@!B`E:?üž×¬#ßÙ?áò_£Ô†?»ãâ½úÌå?ãe	ÚtU<@éBb{[?î'ϝ+õ¿èWrþ$]­¿ìJ-J»æ?Óºí¡Ç¿Õ yó$÷¿áâ"I΀+UNASNone?ïþÇ~·ÉŽ?'qõQ'?#ˆä(ëÝ?'qõQ'?ïõÁÿz…=?T蟾Ý-?T|J.T®?T蟾Ý-?ïèëFÅ?l,ffl•²?gëùӋ?l,ffl•²?ïûQËàÏÊ?0i¯:e?B¸Ï~ÄÍ?0i¯:e?ïþÁ0âK?)Úá
Üt?#ìó™µòÊ?)Úá
Üt?ïׂ©¤9í?|]¼Î$­?t>«F¡È?|]¼Î$­?ïãrÁœ¹?x<­Ð™?l>‡œ6m?x<­Ð™?ïèRAôÊ ?`–˜tãK?g­¾ÓŽ?`–˜tãKAGN4FGL J0328.4-4736?ï—3÷÷ÚÀJ¢s-õÑÀ:ƒ®E"IÀ<µ÷ڗ«@b±½|ͱ@¨¿§J\?¸ÚÇ6_ãj?"O®ÐËS?Êß«6Os@´Íí^<Ì?Ñ£ø'Äj¿âõmÕÆp'¿ça"oŽ-¿â¿§µ¼¿àá:þϾ¿ïÿþR€ÖTUNASNone?ïþcöÓ8?A-´Xh}?)À–@ën ?A-´Xh}?ï÷¿·KÂ?R·ð|'¹?Pà€·ä?R·ð|'¹?ïö7³[Ⱥ?J¨üØ}3?S™SmLI?J¨üØ}3?ïþ¯Édk?v®¬R?%h~ص>?v®¬R?ïþ|G׸—? Ä"(Y	?(;…•ƒ¶M? Ä"(Y	?ïݨRL±'?w-™y?q+ÖØ÷Jø?w-™y?ïõÙ§nÞ?V6ó\ݔY?TMz("?V6ó\ݔY?ïüÛ°•_?1"#L².!??™#ÖÇ"¬?1"#L².!AGN4FGL J0328.5+6114¿é0enLls@`'ßBñÀ9¼.±Ä2ÊÀ;wÕ<ÝÖà@¼®'úï@í`Á
ø?ÇV–$D-?ËÕü3Ã@B`Û*±@ÂÅ(=¶Å¿á¥‡
¥Úð¿·<Ê5ñE¿éÈ>O¿çÁ‰¢«'¿íÒEb	àT¿ï©œQ3¤UNASNone3FGL J0332.4+6110?ï0©¸m?£·ž—y<?žêʪ+å?£·ž—y<?îýËÐ?£TÑ/'Ü? #Oƒ~'Å?£TÑ/'Ü?îv½+Ö.?˜$MØ?¨žT0²9?˜$MØ?î¢èµ"<?ƒ‡)zXÔ?¥Ñt±•ªE?ƒ‡)zXÔ?ã¬/n»A?ËN±Ú¿9ø?ا¡#ü‰~?ËN±Ú¿9ø?æ5wüÄiÚ?ÏF€àî e?ӕw,K?ÏF€àî e?àõ ÞhŠ?Á,SðíéR?Þ¾CÙ.ì?Á,SðíéR?ãg""A÷$?µøEqÈF
?Ù1º÷|¸?µøEqÈF
AGN4FGL J0328.6-1129¿ï‹]v}µ¸ÀHü«`kz¢À:Òe1³sÀ<"½	á*R@ONœÆ@)ÑÀQ"G?÷:ÿ°Nè?'–¶q2?ϱ^œÃo¬@e-a4l?Ï´UªV€¿è—ñXP¿æ?ªºÔ¿Þ墜!´0¿éÙßÚƋ?ÑZ½:ÞxUNASNone?ïúô	ý"Ñ?@"ø€-Êõ?D/ز³&ˆ?@"ø€-Êõ?ïöQIÒ:?SЛ$:rD?Rá]ó;÷?SЛ$:rD?ïé£íÞ?`ëøþƒO?f\þêF|\?`ëøþƒO?ïùÛPü¥`?0àUÉ,=?H'»Pىø?0àUÉ,=?ïñsöû‰?V)›ih?]þí@?V)›ih?ïØãÂb&?xn~Yír7?sŽË̸?xn~Yír7?ïà›S~ò?vhˆ™Zô1?odr—ãf5?vhˆ™Zô1?ïá¯x[¹î?]î¿~ñ#?nP‡fm«?]î¿~ñ#AGN4FGL J0330.1+5038¿ç'"ôéBòÀÉHýŸÓÀ:!2m:•þÀ<º«bú@Ó4E@äÀ§$?ÄBصä(?Øü;Ú÷‡á@n¡žJÙB@Ú²šF'¶¿Ù²^ç0¦¿Ö¥›E]à¿ãí¿@r5ý¿ã•#þŒãS¿í«&[´\¿ïµëÿíáoUNASNone?ÛÂv"khj?È©Mìœ÷?âĶJKË?È©Mìœ÷?åKH°æ#?ʏ!毡ï?Õioþž3»?ʏ!毡ï?ãÛ.Øc6?³¸Óº:?ØI¢O9'ã?³¸Óº:?é_	?Ÿá
''?ÈEjƒ£Û?Ÿá
''?©Gຠ"ù?¤CûáÅÿ¿?îkô"ðp?¤CûáÅÿ¿?ÁQƒ¾™‹à?Å´òÕ8ñ?뫟Y?Å´òÕ8ñ?·N14'?¥´Éî—™?ív:i|?¥´Éî—™?Ék…µ:?©\áÁ÷<Õ?é¸e'½1?©\áÁ÷<ÕMIXED4FGL J0330.7+5845¿áâåy'Dy@-Í9ÚÀ9wb§•À;4ž"ºåD@~B¨œ@a¤_Æ9?ȈªÉlÅü?Ýøk¡Ž°‡@h£?4É@3:·áÙ#¿à6€d¿§ŸÑþ =¿åÔÀdïn¿ï6ci[ä,¿í"äEV¿ïÿç<t%UNASNone?è3¿n%³ª?Å=|È?Ï1Gi1X?Å=|È?ԃ':n©?Ê@ýMjŽa?å¾6âÈÀ+?Ê@ýMjŽa?æYKÛ˘D?±kŸÜ
?ÓMhHhÏw?±kŸÜ
?ßì<K,E¦?­=Ν«xÉ?à	áÚiÝ-?­=Ν«xÉ?Õ=bYšÔ?Í:Úos?åaNÓ2þ–?Í:Úos? Ì³çír[?¬ó
æW˜?îó4ÁŽçJ?¬ó
æW˜?н˜Ó\D5?²ÜnPQç?ç¡3–QÝæ?²ÜnPQç?œåK$¿Èš?"gʎ^ö?ïÕ§û{?"gʎ^öMIXED4FGL J0333.0-3044¿èPQÞçMúÀKRxá"-oÀ;MœÏڞÀ<Ø´*>—ë@FdV@Ô\?ÿ«[˜­
?ÇSÀÜԁÍ?ªhm&ÉîK?äÏ Ä0@©CU,¿í¦M;òõV?ïýR¦–_¿á:ª‹Ydö¿àH?xæò¿ç/jñæaÉ¿Öф!bPWUNASNone?ïÿ~%}p¢?½HiQ*?;RÝ¹í?½HiQ*?ï÷KNï¤?S+U"j.j?QibçøH?S+U"j.j?ïöêf!j?BÞ2ì4ž?R+4.®ZÆ?BÞ2ì4ž?ïþH"´:?Ú鶁]?+}àûg¥˜?Ú鶁]?ïÿcah©?ÛÕQî²N?"×
›ß?ÛÕQî²N?ïÛ(Âc^Á?xAz(ҏ?rkžãž3&?xAz(ҏ?ïó‰4Ðï?d™g췜?Xí–eA4?d™g췜?ïúÝêG?9¯j'×ýš?DˆWHW"ç?9¯j'×ýšAGN4FGL J0333.4-2705¿éªÓ>g*ÀK¶"‹ë[À;=`ðà:À<Øꭈcç@K¼À('?ÿÆü9¡â?Ê}v"q?®†‡™'?äh][Œ@ôôÕ)"¿ïŽÄ¾áQ¿?íôÝ!®¦q¿ç <4cµ¿Ä{ÿÀ?пåÝÞ!ÞÌÿ¿âÆV@~uQUNASNone?ïþù×`¾K?Ï2'˜
? bˆ/¥Å?Ï2'˜
?ïö*#ó'Í?V|‰;Éø?S«¸#ù&™?V|‰;Éø?ïó¬­üÑ?S9ù|k¿?X¦¤h+lÓ?S9ù|k¿?ïû¸y{?+'Ê(¾ï?CƒþtC?+'Ê(¾ï?ïÿ1Òºu?0Z'n?žïw°V?0Z'n?ïÖL
°ÓÙ?z";•­¨Ò?tÙù"³|?z";•­¨Ò?ïõÕÞTšÈ?`úÅ?"e?TTBØXÐ]?`úÅ?"e?ïìDÖìé?WeSˆXÎ?c»)Exw?WeSˆXÎAGN4FGL J0336.0+7502?Úö NB@/DêÀ9ŸÏ!:ã+À<Y›0r@\kæ­ô?ütàaÕ.?¹	àÔk§™?ُ/Þ?@ 	ó蚈­@LŽ\¤œ?á%âØo˜¿ß¬übf§¿ÒQþ$ˆ x¿áQ"²ªØ¿í*ÎuCxü¿ïý/k'–GUNASNone3FGL J0336.1+7500?˜ÚÞÍ?¦	áDòÛý?ï?o¹mÁÇ?¦	áDòÛý?ÆjO1Ê?Àµ5'š2,?ê|ål3?Àµ5'š2,?º•³Ä?§³i-Óé?ì­_Üßiˆ?§³i-Óé?É#µãbv©?«'сítp?é·‡'bV?«'сítp?s¯*À=f? qeeX¡?ïØ¡ª'ÃÅ? qeeX¡?¢ðòÊLØ?¤A){Z†?îÐðӒ8Ò?¤A){Z†?"h£y?‡¯Ý×ÜË?ïdºçòíô?‡¯Ý×ÜË?Š¾ñTÜõ;?y´ŒþÅ\/?ï•:'K?y´ŒþÅ\/PSR4FGL J0337.5+2423c?Ô;¼9ҎÀ8½ëcÉÀ:¨—,ÊÀ<E»,'X'@#:´†ÚÐ@"WæpâÁ?Ç}–™4?Áo,ž¯N?öŽÞ9ܚ @(Àr×
?ïï"b*—ƒ¿Ù£`rpá¿åSj
_Õ¿æzˆ\Zsê¿áåO_¹£û¿èӎg.UNASNone?ïýpcóÍö?+#þþ0"?4|ßM–ä?+#þþ0"?ïô(¾1 Ù?V}´'?œq?W®ƒ,?V}´'?œq?ïïYŸâ´?Z—é$?`¦_ëæ?Z—é$?ïê_ÌÄ>?D©Å"~É{?eb ?Ð?D©Å"~É{?ïõ2éٚ]?SšòZ¶?Uš,™Â…Š?SšòZ¶?ïÐÇ`| ?~Ô!©Ë?wœs»$?~Ô!©Ë?︖×>ã?"û…·?ÚJ<MÞç?"û…·?ï}ãAÙ?xi˜ˆ?.µ?Cœ½ŽÒ?xi˜ˆ?.µ!AGN4FGL J0340.4+5302¿äÐD<'׿ý&^ê–À7½?R%gÀ:ÂÊC…Î@ŽÛö¶U<@Àìœuìì?°¸q`•l
?äéÝ~Ë·ú@*Q)®O3@ÆÂûè™1¿½2t†¿ãˆnßßh¿í³k¢Š¿ï"Ú'—õU¿ïþT~ÝU±¿îmõa™šUNASNone3FGL J0340.4+5302?¢ä9	'Ï?²ñ43
Œ?îÞ¼Séó?²ñ43
Œ?®IÃöÿ,?¬˜ÿgj!¦?îcÀ'!?¬˜ÿgj!¦?ÔR‹Eª?¶apæb™)?åÖý|º]+?¶apæb™)?CVVoE¸?8ËJ¨aé ?ïû*wð?8ËJ¨aé ?ፚä-¢·?×é€R±äÐ?ÜäÊ7¤º"?×é€R±äÐ?'¾ì¿±Ø?‹Ë–v6"?ïµMäÜ°?‹Ë–v6"?Ú"z¦Û?ÅÓït?âî¬ý?ÅÓït>¨Øj€T¶ì>¬\_ý¡bÁ?ïÿþr·,§>¬\_ý¡bÁMIXED4FGL J0341.9+3153c¿ïÿúýóÇtÀ2]`—ÌÀ:4NƒÒÀ;mœzª@/¿@÷C[Ÿc?ԞLœ:Þ£?ÜÏí]æåþ@âyWòÔ@\ò´½âN?å¹ÛÃà•?ÜÙ&wc
ì¿Ù5ä=Àµ¿åÄîs¿ïýà€ˆÑu?ï©ïÝÈóyUNASNone3FGL J0342.3+3148c?î+?mº?©'r–¸x3?¯­NžœÙW?©'r–¸x3?î8×G­œ9?³y2Ó´??¬r‹¶ |?³y2Ó´??êŠ.a^·?©‰
‹aW?Å×Fz…#¸?©‰
‹aW?íjþ*ÉB?™Á»$BzZ?´¨¯ùµí?™Á»$BzZ?èkï×?Ã+D F%?Í¿'P@£ù?Ã+D F%?ßsá}w¾Â?Ò¿Ö!è¼?àFAD Ÿ?Ò¿Ö!è¼?Þ	ß÷@?¹™_¤4»?àûs"uà?¹™_¤4»?Ýõ·¶©ä"?ºˆx›-~¥?á$$«
¾?ºˆx›-~¥ MIXED4FGL J0342.4+3125c¿í…)Ü-¤À2©Åæÿ}úÀ:Õ@8ÕÀ;x=õ.æ@N‹Ô4@J·'$1?ç&
{ÅÕ?Á6fC€Þ7?û6jŠ¸UG?î`
­¿&­¿Û›ã`bt¿ãôw JŽ¿éÙȓ'(d¿è«Ë*5]°¿ÐÝg#Д­¿ïóy^æ•KUNASNone?ïҀ
Š	â?¡@Ý£†BÕ?v¿ùW'Ú¿?¡@Ý£†BÕ?îçåàw­?³Ç¸]K'?®A¡ž0?³Ç¸]K'?îËoWÚ:&?™U¾õßðµ?£I
'\]›?™U¾õßðµ?î随|¤?G˺‹Ô?¡fWYؽ?G˺‹Ô?íÑ1÷Úþ¥?»ú€1‹¾?±vp?Þ0Z?»ú€1‹¾?ßþÊJUu?ғ)âÙ?àšôÚÕF?ғ)âÙ?ëü¶}Æ?°ö@ñÇ4?Ô
&àç?°ö@ñÇ4?àkdIx?Ç@]#'Í6?ßû)7mß?Ç@]#'Í6 MIXED4FGL J0343.3-6303?æ½ì$´rìÀFF	=–c"À:Ÿ–€	¥›À<¬F<$s}@Á²2l¹½@b°~¸lÃ?¿Ù•2+Ì7?©wDã'i­?ë™þ^?Px@¨S¢ivç?îg‡=¡v2¿çÍMZü¥Ø¿ßçÚ$#JÞ¿ä~q f¿Úiœ;_|'¿ãTÝ<†™UNASNone?ïüA.?.¤	ˆN?=öŽ{Ôâ?.¤	ˆN?ïõ·ZÛÔä?TøxEow?T'JiRxw?TøxEow?ïñKZ­†È?VWPú9†¥?]iJ—4ç?VWPú9†¥?ïõ®´è?:Êla8B.?T£Ý³Ûd?:Êla8B.?ïõíÀ7h!?Kö†—?T$¡­Ýœ?Kö†—?ï×ì;/´?|…eõp6¡?t	â"R‹A?|…eõp6¡?ïó²&$Ï:?g–LùÓú?X›³P­+?g–LùÓú?ï×LB¨,?b"¹™½Î?tYó×ÅÕ?b"¹™½ÎAGN4FGL J0346.2+3235c¿îÌ`"à^À1?&9O¬æÀ9ç"gnÀ;ˆ®¬Ÿ0@À}ÆC@FÃ1B˜?Ë=+¯†?Êr)H!@Y)Ù‰t@«;[ º ?î/ŠÂ;N`¿Û!ª	SeÙ¿êÜÕÃìS{¿æàáVÈ¿ê3Òê¿ïq"L["fUNASNone?ïÝ÷?n'û~;É?qr}|¼?n'û~;É?ïÈÿŽÒ&?'éÚ¨nOê?{€8‡"ˆ?'éÚ¨nOê?ï]¿±0d!?ˆÑåþZE?"H	Ø;­æ?ˆÑåþZE?ï5ýPg?ug'FÚ~?™\€^Š$?ug'FÚ~?í½vîýVá?±]ùEhÏS?²H†Ënz?±]ùEhÏS?î˜UÅÀz??±#¥6/çÏ?¦z£§gø?±#¥6/çÏ?è®Qù‹¶q?´…Ë	íÙQ?ÍF¸Ñ&=?´…Ë	íÙQ?è>eÑk%?­7ˆT
M?ÏhºS£k?­7ˆT
M0AGN4FGL J0347.0-6400¿¤:£E
'ÀEÚà"'À;¼qáÄ«–À=_@©={Œ@?²õ`>Ú@D@¡±?ÔaÝÖ	Œq?ïpaêh@¥€éŸk@óĺÇ`¿ìolÕp«¿Üޝ"µ²¿¸®ƒ5ªø¿äVˀœ¿ì°<]ÔF"¿ïÿÕ"[ʁUNASNone?ë1>2YˆK?À#6= >[?Ã;6™ÞÓ?À#6= >[?íþî/Q?±`‹Å–Xº?°Æü?±`‹Å–Xº?è÷~hÞT?±³³q?Ì"\‡â¯?±³³q?ê~ºiÌ?§Ø¡‰¶?Æõ[ÐÐ?§Ø¡‰¶?ã6U‹'‡ì?аµp?ٓTèÜð(?аµp?äPU'éT?ÑÓ´yŸ˜?×ç_Tú-X?ÑÓ´yŸ˜?ÔZfè0DZ?À¬k˜ÕN|?åÒ̋çÝÓ?À¬k˜ÕN|?ԍ̧
£?»iŒ¶‡;?幬yp.?»iŒ¶‡;MIXED4FGL J0347.5+0722¿Ì¯ãGˆ>ÀA"åÞÊmÀ;oH-–;@À<šŒq'êS@!'µ~R?üÃ?ÕØå	?×ÈÛîBé?Ôò–'•¿@µŒ>gCÜ@½l‡'±¿ïþØþ^jD?ïÿñ‡—8–?ÙËëü<üá¿ËЎxSMÛ¿ÌØâ
ü˜¿ïû|b§,UNASNone?ïúM^¶!m?YÊICÒ?Fʅ¥_-'?YÊICÒ?ïñôæ¸M?Zäö€®?\3{^u?Zäö€®?ïp[éúsé?'Ž_kÚË?'ô'À±'ç?'Ž_kÚË?ï䢛Ã6î?XWhhZ‹?k]d~Á'Y?XWhhZ‹?ïùž¡¦>?EðÎA?I…zhÔè>?EðÎA?ïÈ}DÙm?'ddî!-?{Á^í?'ddî!-?u¼"c?XßÉ'?Œb÷g3?XßÉ'?§¬+í?ƒ¿U5ÖÉ?ÖÔ<›?ƒ¿U5ÖÉAGN4FGL J0349.6+4026?Õ¢s	.tTÀ%GMƒAÀ:m@OÁßÀ<òö,A§@fdzÔ@ý¡Ä
†l?Ñ\^¥§ÄÖ?Öf.Þé}@;¹Ïš§@,ý ý{–?ã.žxük ?ïç¶}U[¿åçð¶6¿àH"íˆ.7¿ïÿøÞ£Žæ?ëóæ·YžUNASNone?ïLN+Í?™Ûã({?ˆ¬ì\µ½?™Ûã({?ï'=žµÑø?•k罪J?‹°˜H<­ü?•k罪J?îv1õñ^R?–7ŒÏªÏ?¨œàžVeê?–7ŒÏªÏ?îåê¨Þc¬?"§Ä•öÀÊ?¡¡UrÅE?"§Ä•öÀÊ?îÔ.W£¢S?¢e ² ?¢½‡}¨Æ?¢e ² ?êÍÚ1Ø?Écoë?Äȗ;£ø¡?Écoë?êŽhãï(?±ÜUlHG?ǍÆ\pC_?±ÜUlHG?èS¨P8!?´â4\æÑT?α^¿‡|?´â4\æÑTAGN4FGL J0357.7-6808?è¯î(MbEÀDO
å6PÀ;ÏrÎ\À<öòB9`@!Êy»WÚ]?ú6?Ýe¡E?ÖRÆ«ú?À£ÇšÞ¾?붖à+Ï<@J÷ñé'Ô?àq<þ¹?ïÚÚA)•û¿êòø°€eì?Ì®‰•Àq¿æ۝ }Ç?»ñÿPUNASNone?ïÿ#ê#?à7œ<ݘ?'·ÛUº¥?à7œ<ݘ?ïö"  c?U«Ð"ΩI?R÷¿ÍŠ?U«Ð"ΩI?ïán@¿&¶?rÓ÷'‹ñÛ?n'¿@¢Ÿ?rÓ÷'‹ñÛ?ïü½5*.R?)rL"Ó[?:XG'""?)rL"Ó[?ïý#OCÖ?<–¬£tèà?6å…sþo©?<–¬£tèà?ïÚ-âZË?|*Ö°_à?ré?ñõâ®?|*Ö°_à?Ï°Ç?œ:ôø®á?‡<úåÂp?œ:ôø®á?ïõF¾x?O6^ف?Usö\"0É?O6^فAGN4FGL J0358.1+2850¿Äùy~8ìÀ2[YÿOÖØÀ:÷
"ù$À<\ZéZ¢
@°Áü9L@¿­½=Ñ?Õ¤Ùÿj+?ê7H €(.@.Z¡6F
?üÅÈkêó?íÝ	@¢C¿â›EÁ*WB¿â!'o°'¿ïÿýF\I?ïþÞݛ|¿ïÿý{ÁA~UNASNone?íå{½²ö?·Uø#'V?°× ZšT?·Uø#'V?í́GŠ¥'?¾Û?'ƒì?±›õÂ`ùo?¾Û?'ƒì?êЏ®"?¬˜f¼8"?ĽÁG™­Í?¬˜f¼8"?ï»ûˆ™c‹?~Ùblé°±?ê%=?~Ùblé°±?éoóOg?É2¿gUò?ÊC"2Ãæc?É2¿gUò?Øߨú/Í?Ô
»,ܾ?ã+'ÿh?Ô
»,ܾ?àX÷ý@÷±?À:ÿÒ«?ßN~Ÿ?À:ÿÒ«?è{lI;¥?ɸ–ýæ}Ö?ÎN۟l?ɸ–ýæ}ÖMIXED4FGL J0358.7-7403?è澿)1cÀB£"ý*bªÀ;20:ZnáÀ<ˆ0bžZÉ@e[ç1@ÎàV?̒3ž½ð¼?¦òC~ÚÑr?Øm˵u˜3@fâ(~¤K?št.P}¿•²ù#hæ¿ç,—moo$¿â7¡Â]B¿æb§•¿ïí=±¼PUNASNone?ïþ˜åÿú?7Ð3"P?&~rDí¥?7Ð3"P?ïõé3¾Q?V͇mþ3?T-˜WbÝ?V͇mþ3?ïåðk§1Ì?t~c¾Øü?j"Fð;©?t~c¾Øü?ïûÆQñÊ?$¶?'O÷º?@湟w?$¶?'O÷º?ïþÊç"3?™º¡™¯Y?#Qg݄*?™º¡™¯Y?ïØ_´èÌÕ?|Ž"³õ¦?sÐ%sŒQ£?|Ž"³õ¦?ïÒZåB©?€œE;Úê?vöÒsñˆ?€œE;Úê?ïékfîˆ?V"ÙóoÆ?f"þÖêoæ?V"ÙóoÆAGN4FGL J0359.3+3626¿ïá\ü°?À)%òE,YûÀ:…¹ª±À<pÚ]¯@$)*Ü@ú'QT†?ÐtµÍ¬Ç?æÛÊ@«kÔ@êyþɟ?ö¼ß2ªø?ïmíCdٞ¿¹ÄÞýã|¿ç¼æ'æ¿îÛú'½˜¿ïû^°d?îtp–kUNASNone?ìPê—ý§?ÀÏÚ!Ë=?»•x«@È?ÀÏÚ!Ë=?â—Æ–ãî?Ì­ÍQƵö?ÛÐrÒ8$?Ì­ÍQƵö?鸌ÎÚï?­ cIfÖ?ˁÌĔD?­ cIfÖ?âŽ)œí?µ_Ô²Ý?ÚãìÆ$Æ?µ_Ô²Ý?è9³ih=E?Ëîy"‰Ju?Ï2Z_
ì?Ëîy"‰Ju?¶d't¬?ºø{{9m?í3{Ä"¯?ºø{{9m?ڋT…F"?¹-îwÅÈò?âºU½\þo?¹-îwÅÈò?®$Y2˜¥ö? q€£b÷ð?îºl'½q? q€£b÷ðMIXED4FGL J0403.3+1249¿ì	7ÝDœÆÀ<¬€"ÞÀ:èù@ÉìÀ<'ä™r,@VŒè±.â@?)á{?ÀӚÇA«¿¶ QY9S?ö̯UÀô?ú®ä­³,?ì0©€—j¿ê;÷'X	¿ÞH¿nÀR¿éÐ"¢lQ¿ÑvÒîL#¿Úé<+)UNASNone?ïü_ÑÄ$Õ?:pA'Äz?=oÈ|Ü?:pA'Äz?ïå³ìCÈ?q6-†ôlù?jLÝ` …?q6-†ôlù?ïÏßq<X?{NÔv¬?xw¬"à?{NÔv¬?ïåvó'?UïÑ,''à?j‰'
]??UïÑ,''à?ïðŽ?]yöíÛÛË?^ãïR,£o?]yöíÛÛË?ï\´'A±P?˜ìÜ}=E?"imÐêž?˜ìÜ}=E?ï©l´D{ì?ˆa÷øâ?…¤ÒòP õ?ˆa÷øâ?î…kalÛ?rjÏ®]ß?§©Iì±dT?rjÏ®]ßAGN4FGL J0405.4-6929?íþÍVp¶2ÀC©= ò¾ÏÀ:'3æÊÀ<q´üÌnÙ@*£ÉO•@mt­P0?»‹/ÉqM ¿˜ßÌȉàÙ?ݺÛGŽŠ@	‹QC>™?ëwA 3fµ¿ædaX"¿éË¢«;-¿Û£J<º™¿í°¥)œ±¿ïÿÿ&¦³UNASNone?ïûåÓ©‹?1žïó•º?@ké]ùfö?1žïó•º?ïöéo´‡ ?U{JèsSÚ?R- ég^Ê?U{JèsSÚ?ïçÚ@7?hÚlõ?h%À½@À?hÚlõ?ïüT¿}Œ?(9Zßì??}[g8?(9Zßì?ïúªFÄö?=a2M͏?EVèO1ïŠ?=a2M͏?ïÜØyÙ?z®Dޘ²'?q"Ȭ¿˜?z®Dޘ²'?ïìsQ—ˆ"?l‹ÿé^ó?cŒ®C[´±?l‹ÿé^ó?ïðò'?nf?M""–AG•?^ÛWçãù?M""–AG•AGN4FGL J0405.9+3041c¿À‰j.ilMÀ/±_$RÅ À:Å><À<
Bð?˜œ@Þg~ê@%
ÌÜ­?Å["J§îò?‡¾%·l	á?Ãî;ÝPÔ@¬G±"?îß"o–Ñ?ï´÷ù¡A.¿ëqM_¯=¿å8׊•ñ¿áýK 'ß¿ØœbÁì!UNASNone?ïöWÓ%¬b?uÛ
ÏP-•?SPYIsl®?uÛ
ÏP-•?ïïJá®8ì?g-›^â®Ì?`µWFtl?g-›^â®Ì?NÕ?yÛër§?~·&F·†¬?yÛër§?ïãÃÊÖ¹œ?Sƒ÷óvm?l<5)\P?Sƒ÷óvm?ï¿ú«Ïž†?´íµ?€U?Ȍ?´íµ?ïºÙST!&?Œ×"û¢?I«! ®?Œ×"û¢?ïE~ù|¦?'ÌÔHZüj?—\Ð"ˆ9L?'ÌÔHZüj?ïBBÔ!;?ˆ­¿Ä»+F?—·¥"o¢?ˆ­¿Ä»+F AGN4FGL J0406.2+0639¿ç—oRÂ&À@Ô^'…ÏÀ:£Àd¾À;ÿt²G@{Â4moð@l¬#	"?ÓYùñs¿'ѯà'â?ÐDƒEW@ž0ªlЎ¿ÍÑð£Ä7¿ê1[Xo®¿ëñ±¾SF¿Þ—\R'G¿âŒœÆtÃ÷¿Û|c=gµUNASNone?ïü'nCâ?7Ç)íµµº?9Ó·? Y?7Ç)íµµº?ï÷1†Ï?R¬·Ã 1Á?QœóÒrB?R¬·Ã 1Á?ïéÔQ²?lÅòu´?f+êŸ/­…?lÅòu´?ïýh&–(?G'νº?4¾ÌA½ÆK?G'νº?ïôJqµœQ?Xq•òÚ£[?Wkmþ?Xq•òÚ£[?ïÚxŸ¬‹Â?zÎsiþÒ&?rð"Úæå?zÎsiþÒ&?ïÈC7"ž?‰°©'Åv?{Þd8á‹\?‰°©'Åv?ïëEF8Ò?X@o"]¹?dº¹ÐÌÛÃ?X@o"]¹AGN4FGL J0407.7-5702¿ç*`og¨ÀF4¯O
"MÀ;/øIRYiÀ<ºª¤ƒØg@'šúlÃ"@Ù{f¨«…?¾/p[áÇ¿¹‹ä$WM?ûúÃ.¾Y@[ŠPÑSÅ?í=™Þ¸Ý'¿åÉ>ÃNŸ¿æ:V=#vþ¿èw²ß:みæ­ Ε?¡>S‰ÈUNASNone?ïýÿCäÓ¡?#ì&ÆO?0á4¥cX?#ì&ÆO?ïí<˜Pˆ?jåhÑj?bÃgx~#Ä?jåhÑj?ïâÔŃq(?eÎ	?G†?m+:ƒnü?eÎ	?G†?ïõó$FÔ?>úr¨|™q?TÞ©èb?>úr¨|™q?ïúâ[¡³¼?A'D9®‹
?Dv'#nf?A'D9®‹
?ïªx'®×«?N`¦¬ÿ1?…aßPÚyc?N`¦¬ÿ1?ïŸ"ãðÐ?ˆp¡ðن?ˆ7GEãÞ?ˆp¡ðن?ïrû¯°©£?ƒ	ÚF¢n²?' ŠÊ˜?ƒ	ÚF¢n²AGN4FGL J0409.2+2542?íõ½B¯ì±À2à}=B€®À:ÁZˆâ'1À<T3\MÞ°@ x×­{xÇ@#!m8?ƈï-ö?°'ö¸»F?ì2C¬ýú@7;«|Æ?ïï"'`í׿çä‡v¿Ôƒá6]E¿ÓØ-=¥Òã¿æ´Ã { Š¿àPÂFbUNASNone?ïüÖÇÄǒ?1nnÌi?9IÁ:U÷?1nnÌi?ïôd}ùJ?UÀuèÅ¿Ó?W7xV}6?UÀuèÅ¿Ó?ïï'{½2?n¼k'ô?`}"2OØ?n¼k'ô?ïá[ÇüÙZ?NÕ÷WÒv?n¤81áUÆ?NÕ÷WÒv?ïûeø
ê?;óÆ&©÷?BhžZ?;óÆ&©÷?ïÔr'«?|X¼áȉ~?uÆ·\ì Ã?|X¼áȉ~?ïð­$.?sŽÅ@—?^à¥=-_?sŽÅ@—?ï‰/¬@e?t¬Ûóⷄ?´â=¶ë?t¬ÛóⷄAGN4FGL J0409.4-3822¿çÚ½/ÐÀG´éNã'âÀ;
Vƶ2WÀ<D@¡±@ ©"- Ê{?ú~e`¬é?Ó듡ÝàÆ?ÜÈ?xæò@*Ï1+7@ŸPW±A׿å P!Öi"¿î؞ý†¨ü¿°‰%BûR¿ÇìÎ_tÞ¿åg쮤"¿å%Ü2›UNASNone?ïúu½yü#?>{>Û&ób?F)
…v6Š?>{>Û&ób?ïñˆ?BúÀ?Y®€jÞm?\E?Y®€jÞm?ï­|ܹBÆ?€ ?ί®?" ÈѯN{?€ ?ί®?ïÒhxKk?^(ih"âý?v˱"."?^(ih"âý?ï÷m~wn?L]ԆYD¢?Q%û&aG?L]ԆYD¢?ïÆ …ÆþØ?€ÑZ6UN?|¯½8N?€ÑZ6UN?lˆ$¸?‹y¢iˆ?ˆäڇ5ï?‹y¢iˆ?ï$Zpl'=?0
}°É¦?›t±ùNðZ?0
}°É¦AGN4FGL J0409.7+4006c¿Õ¡,Ãàó~À úG²À:'OÐ"À;¦y3Ȅ@ô¾}ÿŠ9@)YE³Æ?Ór½â¤$?滄Üޓ@µŠáoò@02…8cŸ?ïìv`Y‡?¢Â{÷-…¿èòF+]|¿î3¡˜@©¿ïü´%t¿ï¯žŒØÁUNASNone?èB¬«wÆ?Çßå©ùŸO?ϖõMR è?Çßå©ùŸO?âáx›i ?Î	Ü̳?Ú<åÉ,À?Î	Ü̳?éäa3K±Ú?¯‹e®˜tÐ?Èn{2Ñ8—?¯‹e®˜tÐ?ތڧ^†Ò?°<^—²[)?๒¬P¼—?°<^—²[)?Ú<×úÛÜh?ÎÈEM*ïÝ?âá"'Ì?ÎÈEM*ïÝ?·êÆ¡ç?ÇûvX?ëRN|†?ÇûvX?ÓóWnsH?¼`³ª"9?æzTHÆ\?¼`³ª"9?¢'ËB—?‰PùQ?îÖÓO·'?‰PùQ MIXED4FGL J0412.5+6519c¿ê".˜Nú@$c€ÞôÀ:÷e&ËFÀ;ˆ`¾†¸ì@u3Ú¢ù?@±z`ï.?ÕJ*7!?ì~kàùª{@	ÃJ¢»K?ül¶-‡£?ïô´<³¶¿ÑÀa"V¿ìœU•:¿éEV¶ÅúK¿ÞgÜó‹}w¿ðUNASNone?ç۹Ϛ§?ÏÛ¿ïCÅ'?ÐHŒ`Ëò²?ÏÛ¿ïCÅ'?âŒÁ"ø«V?̛N‰"­?Úæ|ö©U?̛N‰"­?ëcæH7Á?«Š#°A?Ãâpfß ü?«Š#°A?ã‰j&åG?¸T×A^³Ù?Øí+²5qÒ?¸T×A^³Ù?ãL…~¦ñh?Ѡ霨?Ùfõ²/?Ѡ霨?·Áʟ§Ï?ÂJŸ*Óa?íÇÆuF?ÂJŸ*Óa?ã´Ö	r«ª?¶ÈwšÐÎ?ؖSí¨«?¶ÈwšÐÎ?­m÷"²N?§FŒ={æŸ?î) †÷ð+?§FŒ={æŸ MIXED4FGL J0413.1-0304?èÃù]ñÅÀB'žùTëÀ:7]à…ç5À<$'sZj°@‹¾‹–v¤@óæfÑÆ?À·©°=?–"ÆÜüMw?Ò¨~oǎ@8™E5ê?ïê
*%mx¿áçKh´€¿ãåþAcøx¿êkGa=‡ ¿ëQƜ1$¿ïÚúWI'ñUNASNone?ïóŠ×'*?a‰ÕÔä?XêPºl?a‰ÕÔä?ïóìJãËc?_ÒtøÜ?X'j'ëR?_ÒtøÜ?ï¶/ŸÞ`?€J<ìDäB?'zt)0?€J<ìDäB?ïܳèü{?Zܖ:áË?q¦s2îµ?Zܖ:áË?ï»ý¯÷1®?ŒÞ5¤?"úüf•?ŒÞ5¤?ïԄ*‹]°?|{ºŽ™NÞ?u½êÙ폘?|{ºŽ™NÞ?ïù×P?"ítb''k?œ=žç¤N?"ítb''k?ïRÕ»ïëò?‹hp°*û?•¥HŠ™‡·?‹hp°*ûAGN4FGL J0413.4-8609¿ÞÃÚ/"À=ˆ]…TÖÀ:ԄÁ›@cÀ<yþ+êi–@U£žU@?ý«>݋a?ԉ¢Á
¡Å?äϺRvÅY@‹ðÜvü@m÷[ÐL?ïüWÔÓ+Œ¿ÉG ½û"Ì¿ÝôÝ5¿è£˜ Õú¿ëJ9ßö¿ïøŸ^›—UNASNone?ïëMºY=ð?‹¾?]'jF?d²E›ÃP?‹¾?]'jF?ïܨÙ8Ò?sŸnÚN ½?q«"Rhéµ?sŸnÚN ½?î²-eؐ¿?'.×à¥gp?¤Ý)¢vô?'.×à¥gp?ï^´[;åß?wqÞNˆXé?")t˜ƒD?wqÞNˆXé?ïŽKº¾'\?'jWjR·»?ŒmLïÌö?'jWjR·»?ï"Y§nÍ?'/õ¡˜à?‹;i'´°É?'/õ¡˜à?ë¾ã<û³ë?¨é2poÉ?Ás0T?¨é2poÉ?íÓé†8`;?›FN\oÈ?±`³Ðb¿¤?›FN\oÈAGN4FGL J0414.3+4522?ÝÈ
lÇvÀVn¡žJÙÀ:ð Â'ÆïÀ<4؇3@!I&uà'?ÿëÕ:Y˜?ÈB4‰´t?:9$A†? HŠ]f@'ݳ$A¿ïþ؝»gJ?Ýy¤{õľ?ïßd™¿æÒ®Žd•¿ß^Ù¿¤p7¿äq`Ëò¥UNASNone?ïý¸ÎÞ0?(Y+÷Ó´?29EԂ3?(Y+÷Ó´?ïï&î>4?kP•:Á?`Ùþ\P?kP•:Á?ïތzÊ?vî¾÷8'…?p¹ök4·?vî¾÷8'…?ïél¶À?T'Ä'[›?f÷"qÏ·¡?T'Ä'[›?ïûN^m?=¥ðC@ä?BƇ‡QÙö?=¥ðC@ä?ï®ß'þù"?"Ϙ};Ÿ?"H}'g?"Ϙ};Ÿ?ïÆnUaö?ƒÍ¦e&Ä¿?|ÈÕ48
š?ƒÍ¦e&Ä¿?ïÇâ&r§à?pۈÖ¤£?|ì¯þ¤M?pۈÖ¤£AGN4FGL J0414.6+5711¿ïgà‰©]@͖ hÀ:nìzçý«À<!¬%XC@ á "_Ps?ÿN-E	?ÇoØ‡Àÿ?¹ÝtÉâ?óîZ¼8¨@gք±€?ï¥]S˜.¿Þ#uP5¿ß¥I»ŠÛ¿Ü("Œ,ô¿Ølª'õé&¿êkó™mûUNASNone?ïüΫ°?2Š}õ8Ö??˜Zë®?2Š}õ8Ö?ïåo*&¼z?r–"BB»T?jÕ éî"?r–"BB»T?ïö¢¿?SíÏ'¥Hj?R»ÔÜ­–Ú?SíÏ'¥Hj?ïâKþÊå†?NqêÎ
ïö?m´I¸"?NqêÎ
ïö?ïû–àñ`Å?6YúGcÞ?A¤|ó4¹"?6YúGcÞ?ïâ9 ?¦h8o$~y?œc®\;˜œ?¦h8o$~y?ïí³´Å<?q»	Ökz®?bôLOZLz?q»	Ökz®?ïìÑ7Ú?yþ£ÀÙ3k?mä!6¸?yþ£ÀÙ3kAGN4FGL J0414.7-4300¿î¸A롓ÀGVìÔªÀ:Ô qúïÀ=Û4nœ–@ÿ
Nãgï@Ü¡Ü^:H?ÆÒv‰Ê?"a(å@I0¾
í)?÷I6W™ƒh¢"K§¿ ¨áž)¿Ýýj#ŠHÄ¿ì"PŸTÄ}¿ïþ‰]aZ
¿îÌhÞæªÄUNASNone?Å«"Ö{'?Ë;Û£TXr?ê•<
a?Ë;Û£TXr?ÑË>;hГ?È/SVᅎ?ç`âK—·?È/SVᅎ?Ôôhe?²8¨'Nßq?åöð|KÍ?²8¨'Nßq?©FxžÜ?Sövú?îk˜vGɲ?Sövú?ȪM_É,?ÔdÂ.è»?éÕl¨
¿u?ÔdÂ.è»?¶&hª8xB?»d:«ç=Ö?í;2êý©'?»d:«ç=Ö?¼§{ÚkñÁ?¦.{$¤?ìk"²È?¦.{$¤?WDx䥬?GÙD(ÜNN?ïô]ó%Q?GÙD(ÜNNPSR4FGL J0418.4-4342¿éb>Kj6«ÀF¿á2µ^òÀ;ÑÅ6ÖUãÀ<îì$·o@"-¡À»¡?ödc§oE2?áw¿ßÔft?ɼŸV?ë~X€I¼b@¹@œÓ4ñ?äÎô?¿ïÿêÁf½?ïûÞ.ôà¿àòF¿2/¿ï1½è-{c?î2þ…°UNASNone?ï÷ÿ]G?KYjÑRÿ¤?PE³ŠG?KYjÑRÿ¤?ïöô,{ø¹?RÈ"×L?R§
î©?RÈ"×L?ï's8m?€ïi±ÖƆ?‹c1ÖüKw?€ïi±ÖƆ?ïô".ŠEØ?LB'mÝ8?VÙ¢¾Ÿ¨?LB'mÝ8?ïú7Æ?Hëµ_ÍF‰?G#¯í£óï?Hëµ_ÍF‰?ïÛÚÒ|—´?z±ÛïM?r–à ¡ó?z±ÛïM?ï;ýµU•f?'V*¯3,?˜€IX¼ï/?'V*¯3,?ï흦)Ü?^IL'Ì°?bbYø€?^IL'Ì°AGN4FGL J0418.9+6636¿ï ZS¹Þ@'¬%XÀ9kÃA2Ð7À<
òPŠ@Q˜âdŽ ?þg:×lc?ºØ6bg©?ظ¤¡µqç@!ŸØ­«ŸV?ûò§b,
?ïÿ`Úá8¿Íù/Lñ ¿Ô9-H7§¿áß¡@,¿íz4y"P\¿ðUNASNone3FGL J0419.1+6636?bI´ÿ!šò?v¦?=ÜEB?ïí¶Jïm?v¦?=ÜEB?¼¬1"Å«?¹`Ö`àš©?ìjyÜm‡K?¹`Ö`àš©?§ÅCí'§?™É‡")?—ò6?™É‡")? ›ýûW ?ŠNkjS¨@?îÿ¦@Œ?ŠNkjS¨@?cYrž–K6?Yၥµj?ï즍Y*¥?Yၥµj?™Å«Mÿ›?Ÿ#""Äøƒ?ï7ùÒ¥?Ÿ#""Äøƒ?‹mº´›Î?~±Þ6e?ï'I0±?~±Þ6e?Mß=Ôx?A¢Lˆ@"?ïø»ˆVÑ?A¢Lˆ@"PSR4FGL J0423.0-0943¿ïþòÐÜ?ËÀB¨'_ét£À:ûPÍwíwÀ<¿:4¯46@h÷9±?ÿþó…õ?Í\i¢Ûâ"?Þït—'e@ŸÜœM©@ˆë؀µ?è-'	'`?»`̞¿Õº˜b¬¿âuÛ³¿íZ·qõO¿ïùì?®ÁŸUNASNone?ì{oÅé6n?ºcª"…'?¼$Ð¶L"?ºcª"…'?ïz»;;%¬?",ÁÚ|¿?¨˜¡2Pp?",ÁÚ|¿?éà'?Š¤?°ãG™üÓÁ?Èc×ñn?°ãG™üÓÁ?îKòâƒ?‡§Ouð-`?«N~mb;Ü?‡§Ouð-`?çù¿¸È?Ã4ZŸ!²œ?ÐÇڎp?Ã4ZŸ!²œ?ìÔ RÕ?ÂeÊn<i?¿I^û…iX?ÂeÊn<i?ωHú«éd?º&LG3ú?è­ÁU§?º&LG3ú?瓯Á	†M?¯TA¸Áƒí?ÐØ }ìóf?¯TA¸ÁƒíMIXED4FGL J0426.5+5434?ïã®uÉ°¹@ûH
[À8VĘJåÀ;(&Ú@èÛ2k71@"÷Ãñ[ø?­€4¡Oùñ?Ùô/|ÅM}@$ãBؤ@ÿ:)Â?ÉÍ8¤û¿×ÄaÄ@6Q¿çÍù½ÆŸŒ¿í¦Á Hà¿ïü¨'Zà÷¿ì´¿ÍhUNASNone3FGL J0426.7+5437?v§ªbñe(?vÌfB¥§$?ïÒ°«GÛ¦?vÌfB¥§$?±Ôز¼³Ù?¯ÅÔ°8?íÅdéc±U?¯ÅÔ°8?͟ÛƒÚý?²¾¡Šm›~?蘉	A?²¾¡Šm›~?‡!ãMÄc?{GuÕ7\?ï‰ãxWL?{GuÕ7\?zJðÓ¸†?{S
ÕÕ?ïËjËG?{S
ÕÕ?†Kµhµª?ŒLW¹¨ÂQ?狀Ðå¤ú?ŒLW¹¨ÂQ?É#LÔL¦?³,ñì}'"?é·,ÊìÖ`?³,ñì}'"?žâÌ1mŽ?¢¶ÌŽÌq?ïÿ#	";?¢¶ÌŽÌqPSR4FGL J0427.3+0504?ו5Uf'ÁÀ<ÁR*o?SÀ9hŒs@À;¹ðŠA7@X'ßB@°†£Ð?×9''¦¹?Ã'ǁ&?þ*9ªE¹H@
j»q/ÿÅ
x¹z4¤¿æia#pÈ¿éÆ3k	¿í\¡V&}B¿ïÿ2 ;IW?çZòʍWlUNASNone3FGL J0426.6+0459?ïþºÇ«i•?")å'a!¬?$S‡&–ÛP?")å'a!¬?ïöõšæ?S$‰¢'­¹?RÌVäu?S$‰¢'­¹?ïÅÁx/çy?y+þºž_œ?}Dy_7?y+þºž_œ?ïøVRO·?;҉Ñ a?M¦è;…?;҉Ñ a?ïüAì"lU?CîNÙ9ÐÁ?=ðŸNx›"?CîNÙ9ÐÁ?ïؼ"ÙL?{U—4…?s¡üeíæ?{U—4…?îýXŸ´µ?—Þnhq9? *v´²?—Þnhq9?ïÃ1ºQ
þ?qò$ùsCÑ?~g"ÂÛXí?qò$ùsCÑAGN4FGL J0427.4+6433c?äê×ä@%'"ÂqÿøÀ:.®ZZÀ;¾@=ñŒ@ìýåžÝ@[yJ]?μ~`ƒ"Š?ÓÄ\:é`@nò[Ҏ®@_îZ;4ß?îA²¢i¿…¨ÛD\7¿çžÖà!t¿ïaMl·ä?«Ò¨²FÓ¿ïÿŒ!áÒUNASNone?ïìXc~&?f³tm°?c§œÂf?f³tm°?ï'ÌTƚ?—2¸qȅš?‹ŒêÕ8œ?—2¸qȅš?î£È‡¡R(?•üƒG{<?¥Ãw…êÝ{?•üƒG{<?ï¾:‰y÷ú?pòxÞ±!?€q]ª}?pòxÞ±!?ï'
Nú~?™ôk;&5Ž?}yo°üˆ?™ôk;&5Ž?éÝwP?ɳEbñÍô?ȋ†#£¦Á?ɳEbñÍô?毗ë½;?¹º1Õ;‡?Ò Ð)΅Š?¹º1Õ;‡?ëÒµ#î>?´×ž/Àø?Àµ+ópG?´×ž/Àø(AGN4FGL J0427.9+3632c?ç²sé}À û`'ŸÀ9'É"\h·À;mθ_W@­ÔI@²U'þ?ȾfØ|-x?×pZ›ü@‡è|U»ô@q1¼'?ïÛʖ'¿Ü‹}At>–¿és"ý}™´¿è‰ŠøìæH¿ïèí"Ãq¿ïé¿KÚÉæUNASNone?î	›Lw&þ?©ïƒ0Ñ£?¯fK6ÕÂ#?©ïƒ0Ñ£?êŸÌ‹ßFÍ?À÷NñæÉ?ŀÍЂäÌ?À÷NñæÉ?ì'œ´I?¢²Þsš)Ø?»wc]µ?¢²Þsš)Ø?é‡ÃÒÁó?¡5?*vò?Éàð´ø3?¡5?*vò?ç(k¥Ú3?Ãï'ó²ê£?ѯ(´K˜ý?Ãï'ó²ê£?ÑQ"ÚזC?Ï=ÀMÚÌ?çW6"4Þ?Ï=ÀMÚÌ?à7šàãÒo?¸¾$SÌz?ߐÊ>8[!?¸¾$SÌz?țTÞîQF?¤‰ÅÉ«:?éÙ*ÈDk¯?¤‰ÅÉ«: MIXED4FGL J0433.0+1327?ãùÙ©îÀ+À6©¦
EbáÀ;8×ôH;ÙÀ<튯@ÎpþDéê?ÿÞ5Ìj§?ÓiÎEêœ?ïÿwåëo@Ìã=Qš'@@¤‹¿êÒ2g[Y¿ïénù²Þå?ï½è=–Žw¿×Àó°fe¿ïÌ&´Ÿ¯]¿ïïNÒöUNASNone?ä
L¤¤\?Í&¿¶T]?×ågÔ¶·H?Í&¿¶T]?ì'k\;â|?Á«Ï¸JÅÝ?»l¥ ì#?Á«Ï¸JÅÝ?åõѱ8?²¦"ñ¹ì?Õ fø\?²¦"ñ¹ì?å³8?ü?¸Ô½ÇvK·?ÕÅ™€?¸Ô½ÇvK·?ßIl?Ͼï`E?à[IÀpüu?Ͼï`E?åñµ†×l…?ÑÈfdýŸl?Ô"òQ&õ?ÑÈfdýŸl?Ú)Åê8 6?¸ªp~Ü?âë
ãïå?¸ªp~Ü?є‹aa]­?Á;iç¿S?ç5ºOOQ*?Á;iç¿SMIXED4FGL J0435.5+3232?²Ù-0a]À$
ƒ{á"À:ºÁ濽À<P[¡çEõ@.v‡›À:?þÑטةz?̍ø%ÁÃ?ØèÒý='í@	ñ9þÿO@õõ•måâ?ìÀäbÈ?íúVrÓ\3¿'Š FJÖؿމlLþ¿êz:Ä!, ¿ï"ž"?pUNASNone?ï5H·²fù?¡M|ò?™VéC"ó?¡M|ò?íÃ@Ë»ï?¶,¢<®Æ¢?³'åú?¶,¢<®Æ¢?î[·ƒ0ï?–6cb|¬6?¦úDƒn?–6cb|¬6?ë5ØK}y? œÛ.4R?Ï(žÒ
? œÛ.4R?ìr?ÄÕÌ??µdãI/Æ?¼nÙQž?µdãI/Æ?åÊ,®)®?Ñ'Þ¸©ø?Ôk¦¢ý¬¥?Ñ'Þ¸©ø?çV‡dýt?¸1Pß?ÑÍRñ6?¸1Pß?ॾ­7Ú?»)}8 >?Þ´'¥ÙL?»)}8 >AGN4FGL J0436.9+2915?ԖY@Á™ÆÀ'äAVâdåÀ9ÐϟåãõÀ;wˆ4íG—@3·EQö@Œ²`9ü{?ÁçZS<=?ÎbZû¤&@ú¹o!÷?ðŒ+$U?Öº'#'à¿à·n=h¿ã|¨Ý"U¿áüî
ö¿îLb-<¤¿Ø1Æáü3îUNASNone?ëÏ<ŠŽ¨"?¸[r˜|M?ÀÃ
ÕÅ]±?¸[r˜|M?â´×Á¯?Ëa¯>éÂ?ÛƖQæ|¡?Ëa¯>éÂ?ëøÑ©ðÄ?¦38ßÂ?À¹X? ï?¦38ßÂ?âÏÆV»ùk?«jÝ%‡?Ú`sRˆ
*?«jÝ%‡?ÚSYYô¤=?ÆЉm°Z?âÖSS­á?ÆЉm°Z?¾°ÅÛ?Â:Ÿ$ë>I?ì<©çD>?Â:Ÿ$ë>I?Ú®¤Ëlš?¸g9y?⨭šqI³?¸g9y?¬Vñü¢¡'?ÀòñF B?î:àš˜?ÀòñF BMIXED4FGL J0438.0-7329¿ïŸ
Vg$ÀA—ŠC»@³À:n¢‰,dÀ<}ƒêXÏ@ ¦'æQ?üADˆÆ¿?ÁÅøâG]?´P°Çˆ•:?ó°¹÷2ú@¤h$V¡w¿Ü½ò%Kê¿ìI‰¡Sø%?¢GŸë‡¿ÙàP7Oøf¿ß\*Ãx[¿ßd3›¸Ø¤UNASNone3FGL J0437.7-7330?ïþxµ¾?%¬q¨Ìÿ?(t®8D7?%¬q¨Ìÿ?ïöd[²P?V‡¢¬?S7ÀþcÐæ?V‡¢¬?ïø²8/¥?JñŠ\3+¥?M7Ç-Œ™?JñŠ\3+¥?ïø-]—q?7{'GÄGÉ?OÿJx—_1?7{'GÄGÉ?ïýöHyÉù?%…˜Êø?0M»;eÒk?%…˜Êø?ïڟã'a?{·†á#z'?r°!j+Â?{·†á#z'?ïûÖt/@¤?Vnóg¾º?@¦.ò-G?Vnóg¾º?ïè§ËOc?Y…Õð•?gX4±üԊ?Y…Õð•AGN4FGL J0438.2-4243¿ä#äß>ÀDø¿p]À:¾Ú`3FÀ<Lð\@D&äpX@g ã¥Vf?Á"žy_g¿®	§ô{<Œ?í®"áÉ´@¸"ŒòÂ*?äYo<νh¿ê$DîFš¿æM™{f¨¬¿ê—v©ªˆÕ?γŠ›úÇÝ¿ïÿæ4|ßOUNASNone?ïû€¦x ?at];A¹ý?Aýgw"A¬?at];A¹ý?ïö}É$Þ?SϖØS{™?SÄ@äÿ?SϖØS{™?ï×éq¯V?vQêhŸÝ?tGöh@?vQêhŸÝ?ïþ¬¡fË?)Áh)Þ?%5éÈ?Ð?)Áh)Þ?ïõlÈ͆(?TW'՗+Â?U&nF· ÷?TW'՗+Â?ï×ÍfRV?{ƒ÷P˜ñ–?t}Ƨ‰9?{ƒ÷P˜ñ–?ﶕ€å?ƒ	o ©?'Z¾äîö?ƒ	o ©?ïîçcsdH?\KµÈê¹?aœn_(
?\KµÈê¹AGN4FGL J0439.6-8322?Ù²ó¥Ý'lÀ>•Ëeè'À;%Y>_· À<€RnM@"wïвà@ˆ:Ùð¡¾?Ó?Õ"[ʁ?ÇĕEÌé?ñ(º3m?üNøñ˜ß
?ï÷¿¾€^då¿ãY8œ(À¿âV•Ù¸é¿ï]]ÿ¾¿Ù>Ÿ¿ÎbUNASNone?ïá«ûŠ¿%?i('·Ì%Û?nTQ"ë)?i('·Ì%Û?ïӚƒ]j?z¿|•Çd?v2¾oB'J?z¿|•Çd?ï]ÿhE}?ˆË;ìV‰?"@ùֈG?ˆË;ìV‰?ï£:'֏w?f­DÆ×^?‡1[<²[?f­DÆ×^?ïÍJI‹u{?ufò-K?yZÛPBƒ?ufò-K?ï{¿ÚS¦¤?—Ðû]?ˆº²•?—Ðû]?îC5³A?ý—H`}?«Ç,¥ª'ô?ý—H`}?íÊúš1ç?":‰O"t?±¯8*R‰Ç?":‰O"tAGN4FGL J0442.0-5432?áG5Ò'ˆÀD/§íåÀ:¸8!ïÀ<¨»5˓è@/ëï|Ð
@g­"ãY×?¼ï"ãñ¿­ëþì.¼×?ð:µ´)@v•]ŸÃT?åsú~
òͿ唐æl±¿çÝB 8š¿ç¶Šþøï¿ïÿpޏlð?ïýÕM¤ÎUNASNone?ïû	æޛ×?@B"ªoP2?CØd·á?@B"ªoP2?ïóN";­ð?`]Ã"Û?Yc»³!
?`]Ã"Û?ïэ­ÁÞv?vrèæíï?w9)A?vrèæíï?ïö#¦š«?AJ,ø®Ô?S㸲ʩB?AJ,ø®Ô?ïõñ|b.Ò?UjMùuˆÖ?TüiŒ§?UjMùuˆÖ?ïÆP`·ó?ˆŒ&~ã)?|×Ïų¤?ˆŒ&~ã)?ïÒÛ§†Z?|÷A6ù]Ç?v',"'ß ?|÷A6ù]Ç?ï›[慰"?|Ӎ{ì?‰)PÕo.?|Ӎ{ìAGN4FGL J0442.8+3609¿ïÔ{uþE&À¤¡4˜ŽÀ9×äQMÐmÀ;ƒÔA5Tv@QBŸ@f1rhÓ(?ÆjEî÷š?Ño§BN¯@*F"bH@ªÆ>¾,¿ÉEø\Ȃæ¿ãß¤¬ó¿è€fAÓ_
¿í¤]­Z@¾¿çIžÚv.¿ïì‡b_p©UNASNone?ïÐÜ~ÿ?u{8xs?w'ûÎî"6?u{8xs?îkò×Dí<?«rš}(2?©@ҋ±,;?«rš}(2?îÍj‰??"š˜u–ÕÑ?£)Wp·õ'?"š˜u–ÕÑ?îk׏"»?‡©BÙÔD?©B‡›I?‡©BÙÔD?ï@°âéø4?—äÕ	庍?—é㝙{?—äÕ	庍?ࣁ‹/S?ÒT‰'†?Þ¸üéÓ¡[?ÒT‰'†?ç• nh%?´÷ܽR(?ÐÕ¿#/ɶ?´÷ܽR(?ÞKüÛL0?ºm¾}n?àÚu'Yè?ºm¾}nMIXED4FGL J0444.8-3514?Ô ×œÅ¯2ÀDçÝÊKÀ;k%ÈçdÿÀ<Ëå+hc—@sÆxIè¬@®'r—Í?Ð!DÚ$¤?°g3BE?Ü´_c@ý'öÛ?ïÞ43
s†¿ÙæFñV¿å"ÈA!ÞL¿ïýàÀõ~?ïàŸ°4¿ïñ$ЙàçUNASNone?ïÿXÞša?v—¸£2?äBâ0¬·?v—¸£2?ï÷®£I¤A?RfæD<Lç?P¢¹©0œÊ?RfæD<Lç?ïʘr'9Ö?ä©îì~c?z³Æèóy(?ä©îì~c?ïÿàÙÛ9]>꫽ó!¦">ï& éô^p>꫽ó!¦"?ïþÚ[U¼?( rðûñ~?"ZH$jš?( rðûñ~?ïÜLbìP?z—ª'›–Ç?qÙÏ&ßÝ?z—ª'›–Ç?òÄ?Š•û‰nk?‹YºË1[?Š•û‰nk?ïþµ_ÊV?(:q¾zÎÏ?$ªaL"%?(:q¾zÎÏAGN4FGL J0445.7+1535?à[µ2|TÀ2ìUC(s½À:FE­‰:§À;·áñ÷ÿ€@ĆØ!@Yx"væ?Ó0p ¦ÿ?ÜBéŸ"w@	˅¤ð@ÐrùòŸÅ?Ѭ9d$­¿áËF¿Ä§¿èO¬½ã¿ï~µè"¹¿ïºú<q V¿è…™!y¢XUNASNone?ïÊ1p µ"?y+*d#^?zçGõԂJ?y+*d#^?î'1Ø%"?¨ÁgjÛ?¦Üâ|^
Ò?¨ÁgjÛ?îPýjñ²Ø?–é<&ôKò?ªð)NQ‰?–é<&ôKò?í‰.H
0?Ñ•£.³?³¶à"?Ñ•£.³?ïRÑ^µu¡?—}Ÿ¿­½?•¥Ô$)áî?—}Ÿ¿­½?â8Å	p'l?Ñ7'hwã'?ێuí±)?Ñ7'hwã'?æ^¸;_~?µ"/-¢Í
?ÓB‰AÕ?µ"/-¢Í
?Ø0¢ùÙd$?´4–}¸ñ?ã箃Mî?´4–}¸ñMIXED4FGL J0447.2+2446?ïÿ:¨ûêÐÀ*]ÌcñAÀ:–8¦ÿ´À<LB‡ö@vWNñTÁ@æYeÌãs?Ò‹eNce?îÕëY€@~¿ù³?üµíbC—?ÙqÒàãG?ïÂQHÇïî¿ÐÕao0º¿êÕTáä·¿ïÿw¯d:?ïñ™À…ì"UNASNone?ٛ>—Ô?Î6O%	ØO?ã2`À48?Î6O%	ØO?ØôîãçµJ?ËM^•ëí?ㅈŽ%[?ËM^•ëí?Ýó.eÑ?´Àæ–uÃi?áhötÍ?´Àæ–uÃi?ÌM0ùX'?­)_Iç¬?èì³ü©ß?­)_Iç¬?±Â-þQ:k?ÃW:äØ\M?íǺ?ñ ƒ?ÃW:äØ\M?²­A' Ív?¶WØ0½"ó?íªWͤì'?¶WØ0½"ó?µü±s@n¤?¢t~³ãg†?í@iÑn¶Ü?¢t~³ãg†?ŠÁmUëZ\?yÆYo?ï"úJßLV?yÆYoPSR4FGL J0448.3+2743¿ãÌ[°!À&TŸ"…^À:³jû÷]À;«Lg·Ÿ>@]EÌ=î@U8áÈÝT?Ï'öüK@?ҝû¾|Òä@*à~Zy@¿"Ë(²Ò?î–éP'¿Â"ž'¨'¿æ[™ï)îç¿êB­#º¿ìùYó'\´¿ïõø	'y:UNASNone?ï·FŠ Nâ?yÅ}]ì¤?'.]Qe'?yÅ}]ì¤?ïµ% ñ?q+*?—?œi_{Káç?q+*?—?îq?š÷93²?¯/¹Êõ.?š÷93²?í«)ý¡Î?Í¿u}-ô?²§Þ¯7
?Í¿u}-ô?í¦1ÏIÇ?¨¡\ŠIm?²Îq†û¾D?¨¡\ŠIm?èPèžË˜Ö?ÉÈ"Ÿ
³?μ]"Ñœ¦?ÉÈ"Ÿ
³?åI˜"$Ô?¶ÉTIÌ2?ÕÁlÎ׶W?¶ÉTIÌ2?᲋FßQ?°j·4gÄ?ÝԚérA]?°j·4gÄAGN4FGL J0448.7-2116?êÓ»aÌúÀB€ýÁaÀ:wSeØ¡íÀ<láçDò@^¢›öÁ@‹Âßä?Å,ËåòÍ?Áǎ^ýçL?÷ÈÙm²‹@Y>:"e±?ï¢1þªÀ]¿â«¼|±¿è¢R_ô1k¿ãinX£/E¿ï½vþ«¿ïð­aÍzrUNASNone3FGL J0447.8-2119?ïü'öùWV?1Åb¤d[U?;hIŸ˜?1Åb¤d[U?ï÷_zw?R})ìû{?QAXµÿ?R})ìû{?ïéÝÕ?[
'T¥ð|?f"ù-çž?[
'T¥ð|?ïú| HÆ?0`8ÊÑ?FÝV.S?0`8ÊÑ?ïûYr덋?@åé}®hË?Bš3`rï?@åé}®hË?ïÝ(Œ]"P?z•'¦›Ã?qk¹ïrç›?z•'¦›Ã?ï،òIçˆ?x²ö†rn?s¹†ÍMËò?x²ö†rn?ïí²éû9?PL÷Êòë?bMo£®x?PL÷ÊòëAGN4FGL J0453.3+2843¿åd_®™äÀ#
çöô¾ƒÀ:3á @è(À;¿p¨È@ÅXQzÆñ@%ن³U?ÈVãçp'?Ñ®äïÙAO@»Ò#Mââ@ðßP²ö¿Ñ=˜|c'î¿à£'÷Ó¿ämä£P¿éæg"N¢¿è4©TøÙ¿ïøT<jUNASNone?ï÷xl£Ac?MWCï Yó?Q's9B?MWCï Yó?ïí	2®¨õ?býN±2?böÍ,;BÜ?býN±2?ï¡æ¸8ôœ?£Þ½uKó?‡†Qü¬ý?£Þ½uKó?ïá»=Вw?P¾YÛ´…?nDÂD1\?P¾YÛ´…?ïáñ%þC?nø9»??nÚЦå?nø9»??ä*.?"üøhÐÜ£?‹PÆõzôq?"üøhÐÜ£?î6Kª^Ÿ?U+õ?¬›EV¦sÕ?U+õ?îçJ"I<E?"jçi+?¡‹]Ýÿð©?"jçi+AGN4FGL J0455.9+6757¿º¦»¿o}@.NޗÐk¾À:ô§vÑîuÀ<·ö:"`L@ ‡y{ Ô?ù¦,ƒì‰?Ó#½¿"©@?à¸æÁ?¥Ý@€':O‡'?÷ۑنĀ?ïè;B¡:M¿íÊJ µ'-?³Ó6sXg¿ÓÏF0Š¿éBas7…¿ß?|žJ®UNASNone?ïíX}<
D?aGÉâq'¯?b§'ÅR"&?aGÉâq'¯?¤~,´?ªã±Jþ:Š?¦v´­˜À?ªã±Jþ:Š?ïgµN‰ƒ?'´QÅD˜?œS	]‡?'´QÅD˜?ë3˜`‰' ?¡ùmzþš?Ã1ž}Ùõ?¡ùmzþš?ïY"À?"ÕBx[…?ˆ©hº¿ß?"ÕBx[…?çßåÿÏ®?ÍÆZ­J¦l?Ð@5À`£?ÍÆZ­J¦l?íñC^œ?¡›Q´L"?°uçæ«0 ?¡›Q´L"?âæ豧#è?¸Ð¡—L´Ð?Ú2.œ±¸0?¸Ð¡—L´ÐAGN4FGL J0459.7-5413¿Ïn+
Â,ØÀBíZ[–(ÌÀ;Vµ–Ob>À<è،ôo©@û¾Ù6?þˆw'î\j?ÛCú*Óé!?¯9X';§ ?Ðú`ƒÎV?ùêmÿâÎÂ?ídÈÁû7™¿î;.¿±q¿™]©&¾8¿ËéÙøÚG¿á#[NÛ/f¿ïÿ%ålÖÃUNASNone?ïþr²W´%?¥ñ ~!±?(Ô×dKî\?¥ñ ~!±?ïôkÙÿ:?Z­yšÕ"¬?W)ø6d?Z­yšÕ"¬?ïå~eûKT?qKєіˆ?j™ðò?qKєіˆ?ïïðEwÙU?Dè7†˜‰?`ºzh:¢?Dè7†˜‰?ïÿ
i»ZŠ?ë»î·y?²ÈdMè?ë»î·y?ïÖzÐM,P?|ºâñO®¬?t—ÐzÜ?|ºâñO®¬?ïêt›'Ö?q+äQÿD?e‹dòýÉÔ?q+äQÿD?ïÏqLçº?hq §c?xGq÷Ȳº?hq §cAGN4FGL J0500.9-6945e¿ÅšH~|RÀAeÕQ֌À8¨7æ÷~À;v8è†@~ÕØd/ª@Óo1?¦+±^²<ÿ?REbåÇRa?³WÔþ©c@=`4H1?ïçë ÊÐÉ¿Þ[]‰H¾¿ã»üР–ä¿àô÷Ãñ[ø¿áF]v'Ï¿àïኟUNASNone3FGL J0456.2-6924LMC-FarWest?ïù‡ícŠ??ƒ¨)ÕÈC?IàK6§ý¾??ƒ¨)ÕÈC?ïöS‹\.?V…D]â
C?SùXñ†´?V…D]â
C?ï^ÊѨ‡Q?'­ny	  ?"&¥Î^±â?'­ny	  ?ï梗«>?Z–'ZÃ?i]hE£ ?Z–'ZÃ?ïÕя˜þƒ?qÌÈè$4?u8-Qr"?qÌÈè$4?ïÛ¦ÿU,¥?{cÝQ¬©?r,€veí…?{cÝQ¬©?ïh¯R#Ê?™‹@¯Uj+?ž2ê+"­?™‹@¯Uj+?ïÄ­›*?r·…KYžÆ?}©2"ÎÒ?r·…KYžÆAGN4FGL J0502.2+3016¿ærý7½uÀ+
€òçÀ;)ÿ­Ê©À<7b• Ž@ Æì)Œì?ùِʽþÔ?Ù¢‰bñO?Úìåq?ûmªx.—@,XÛäAÞ?ïÿùëñ¿ïýÅB"Ð?ï}[À›<¿Öèf»ö»´¿Ô©n)©¿ïý'€›pßUNASNone?ïø—çùà?Jêâqö?M _¾n?Jêâqö?ïíÓX4Òù?h'â©wB
?b,§±ÿ?h'â©wB
?ï˜Y²Æ2Ì?…¼'¦¹î?‰é"NsLö?…¼'¦¹î?ïÜè"M?]gÀÙyƒz?qù‹Ä/IŽ?]gÀÙyƒz?ïùÀüη?M[¿Ú`w?KÄüÆd5?M[¿Ú`w?ï¨áIÛu?™ÓÒ@"[ª?…Ç­Ëw.­?™ÓÒ@"[ª?ïHiȒù?ŒÅ#°ë7?Œ-åŸ	Mº?ŒÅ#°ë7?ï²ÃÜ'"?z,»¨jËY?ƒ|•Œ?z,»¨jËYAGN4FGL J0503.8-7508¿Ôò8ržiHÀ@ztBÇû­À;U­…ߨrÀ<¤¬Okx@ÆWÄb&@z…ص?ԏ&#*Q?Ï1¾{{?ñ'ºÄŒŒk@_[]ˆ¿ïù "_Ì?ïúŒž3‡A¿ãb°Ï@E¿å¡"ßþع¿å"PŸTÄ}¿ÚEÙ]ÔÇmUNASNone?ïùéQ¬‰Ð??¹&ÂÙyD?HZº.²a´??¹&ÂÙyD?ïî[CXÖl?fËb7¯N?a¤¼†-T?fËb7¯N?ﻙtÁÚ?uÈõG*d?¢ÌßÕ?uÈõG*d?ïël0f
‡?K˜Ü$Zúÿ?d"ÏÈ°(–?K˜Ü$Zúÿ?ïõõ¼žñ?P˜²¤(ò?T†þ—	C?P˜²¤(ò?ﮥH4³L?"‰™:[íþ?"V­ôŠúò?"‰™:[íþ?ï¹Èáq?".菏ÄH?œˆÆùÔ5Ú?".菏ÄH?ïr–ßd¡?î N"Ã?'­?ìÛ?î N"ÃAGN4FGL J0506.3-0620c?âWŸ¨k2mÀ:6ŠçO/À:¦IÚ>¥WÀ<O%üéË
@©{%2h@š±ý=­à?ËnŸšåt?¸d ,?éžu "se@JÖßuEý¿åEv+ÖG ¿æ0©€—j¿âhx>Õþ¥¿æTÑ]Ö¿ë®IW¿ïûÍÖ¸UNASNone?ï÷¨eàŒ?H§´¼'À?P¯5²Fh4?H§´¼'À?ïó63ÿÈ?_­jcxƒË?Y"—äó,?_­jcxƒË?ﯝC"¡°?~æ¦EW*½?"¯Æ ?~æ¦EW*½?ïè'%ð»¦?MȝpoP?g}ÙÔ+¹?MȝpoP?ïñòklà~?V£Ö~½Me?\(ֈf?V£Ö~½Me?ïÏ)N`"Ç?…ܝœ?xkX°É ˜?…ܝœ?ïŽ+_e|?Œ
0±Â"?Œµ5åÒ?Œ
0±Â"?ïnF"Ä?€
~,#Ÿ?'7-"·‰?€
~,#Ÿ AGN4FGL J0506.6-4629?â6¿Ú¡ÀB{<`ŸÀ;v?""ÆÀ<Ó§<ð@!>÷þSØo?ù(¢› ÚÖ?ÒQ>a¸«?ËkÄIE™<?þ5ctCž»@-œsÇ-¿îm"wú¡?蔩ÀXJD?ïHã—­¿Ý ~Dÿcx¿ÐYGŸœ¾¿ç"…U>÷UNASNone?ïþ-'´­?#lîQie?--ƒJ¬:?#lîQie?ïöWÏc™Ç?TXæ#?SP`¿Ú2R?TXæ#?ïåh'©$?lÑD¦Ü õ?j—ú‹3"Ã?lÑD¦Ü õ?ïö™Ëð·?@f:«Ê"?RÍ<#'g?@f:«Ê"?ïýáhvr3?)oœôh;÷?0ô¼EՋt?)oœôh;÷?ïÙõk?{üSb?szf'R[?{üSb?ïܔ9¶–?wcµØy´8?qµã}óˆ¿?wcµØy´8?ïìNÖ/¨?YÕÎlIÖ>?c±)î¼çÍ?YÕÎlIÖ>AGN4FGL J0506.6+4545¿£5çŸ_L@

Ý8TÛÀ;@{¶YÃÁÀ<r%ÿn	É@"‰ioZUâ?ûŽnD—à?Ö§;®+÷Ö?Õ¥±ÀVò«?òésçXiN@ïÑ—Êâ¿ïÐaò¹F?íÈúz…\¿ð?ïÿþBe«+¿Ó`dYEìs¿ïþpéw'UNASNone?ïóƒ¾C¥¥?€ƒ¸‰ÜQ?Xøƒµ-Ö?€ƒ¸‰ÜQ?ïÕÒî2š?ardå–?uû¨ƒ•?ardå–?ï¥ÇÏ%ÜL?½·<4>?†ŽDG\Õ?½·<4>?ïïî==?SHœÐ%‰â?`ðºþÝ?SHœÐ%‰â?ïëFâ‰ïÐ?dsî»ê9`?d¹4°ˆ?dsî»ê9`?îj»y'?³ý4Ï ¬K?§)THgÞó?³ý4Ï ¬K?ïtñ‹ûû?¸éBÒ¢?'aΧ†"?¸éBÒ¢?ïüåCf1?‰‹ÑAí{?‹ÀÆ«¶×·?‰‹ÑAí{AGN4FGL J0512.3+3329¿ëÚaÔõÿæÀLF__áèÀ:v9´V´BÀ;üz,€@ ŠŸb0?ú–=Ć­.?Ó¥àú¬.?ÜÖÈäŠÙ@æÎãþAº@0@0Fĵ¿áÒ)˜¾&¿ð?ð¿Þ¨'¤W¸¤¿å>8ŸÙ¤¢¿ïúúý·¦JUNASNone?ïôL–d8—?Ra`TÂç©?WfÓ1Ž?Ra`TÂç©?ïÞ4ñ¤G?{dKêÉ;æ?på‡8+5?{dKêÉ;æ?î¶åæ
?˜©_pv?¤'®ò1?˜©_pv?NípS?uñý$'½?,Kƒ#E?uñý$'½?ïã"óÓ³?j'éÏî?lk	ðç?j'éÏî?ïK¼4ñq?¦ïCjôü¨?–Ÿè|Ñmä?¦ïCjôü¨?í{¯=ųS?¥ÔÆ.a¸
?´"†?æ?¥ÔÆ.a¸
?îâµó–n?"ÆJJӘ+?¡Ô¯2ä'?"ÆJJӘ+AGN4FGL J0512.5-2201¿ìíüÕ¤À?êÈ`V'À;&k&¿‡jÀ<~ž43
@‡k;p|@R ÿT–?Àv_'Çp¿¾,8Ã
@³"ý*bª?ú–ÆXêR?ï÷%  ¿åø'Už˜¿ëÝLâ0â ¿ÞµíãðQ¿ìn<ô}ÿ?é¢ áÌäUNASNone?ïøYrY†&?Fœ%ªÂÐÕ?Nš7~ŸU?Fœ%ªÂÐÕ?ïŸVDã½]?–ÔÖMØd«?ˆ*nµâœå?–ÔÖMØd«?曆¸Ž?',tǹý¼?†]ÎÀŠ"?',tǹý¼?ïѹ]Œ×?fSÞK?wt£JZ\¼?fSÞK?ïÒò́Ax?u¥Ú…H/?v†™M͟ý?u¥Ú…H/?êç«í¦ƒ"?ÇS8²à"Ñ?ÄaPIeñï?ÇS8²à"Ñ?ï`N¹˜ßØ?RœEužö?"ö(ÆÍ?RœEužö?ìHf2
?¯ÕgÏfÃ?½¼Ïk‡–?¯ÕgÏfÃAGN4FGL J0524.7-8304?ï3Ál÷À=~¢‹°£À:Mó™À0À<Tˆ'@>Ãز^7@ˆ$&Oö?ÍÛ·`Ô×?Óù|ƒ3Pº@ÿÞr¿?ü÷f³›x¿àHksì`ç?íÁú@£^>¿àJÞ˜–¿ë;›í0ðc¿ÚED"ٖ¿ï÷3rôcUNASNone?ïÂ0*ƒûç?£IÓË©?~çêÏà:?£IÓË©?ïx¨'r¤?"•Â®í'
?êûrs‰?"•Â®í'
?îí-<E¢ï?'
€úÊ?¡-,<¸?'
€úÊ?ï}ó[´?'—Û¯5ޙ?PAžÌW‰?'—Û¯5ޙ?î›DAM}6?¦R»,Ê
?¦K»êLE›?¦R»,Ê
?ìGÀ?Á@É  X?½Ç7ïQÿI?Á@É  X?ꚵd•Ç?°¾2߉?ŕ*m«˜ä?°¾2߉?è9«­ma?µÒF9´'?ÏQJJ{ú?µÒF9´'AGN4FGL J0527.1+1152¿é¶s'i—À)[	¦qï1À9Ó@ŽeˆñÀ;¡¹ìxk@Ì´äxºý@‹®9cÎÜ?ÇV†
JÁ?ÈB¡û'Ýé@-©¼&Œ\@*ø==ù¿ÏZ¡¡¥×•¿ç¨^žEû¸¿çâJãS!¿ék8'ŽºC¿ì.4@ylÓ¿ïÿPþU0UNASNone?ï¾<¢â\p?~߶ €r?€p×C¡R?~߶ €r?ïÕÓ©/ ?zCÖ£v s?usHôÓã?zCÖ£v s?ïC¨f2†?Ž"^û·;®?—êìZw>?Ž"^û·;®?ïŠYm¸ð?mï&÷55?i¤œG—ñ?mï&÷55?íÒò hb6?°˜#¦¤ú3?±hjûsÎ?°˜#¦¤ú3?ïéCê²?¦7b=žn?Ÿâ×¢ª®?¦7b=žn?é7áɑ·?´§"H6–?Ë xÙ¹!þ?´§"H6–?ëU7ªÉ?§8}ÊÓ?«›#ÝTÚ?§8}ÊÓAGN4FGL J0527.4+6647?à
ý!ÜÒ1@1=¼#1]À:ÄÑ2À<¡S¢>"@›_-b
ç@ŸÅoá9?Ãaó$¥PÝ?¯fÿ0ø?ì(›?6 Î?ù÷Xÿ ‰£?ãÞDno¿à_0?ÿä	äO QD¿ßÆæ#5U¿ß¹"@"DÆ¿éÇaS/UNASNone3FGL J0527.3+6647?ïîë½þ¨½?žf yÛÙÈ?aAÞû+8?žf yÛÙÈ?ïÞϹï®?qµZ8ß[L?p˜#Çç?qµZ8ß[L?ïéäEöj'?rÖÒOr?f¹ÿö†ä?rÖÒOr?ï¢òUÈ^~?d'&)=K?‡CjŸld?d'&)=K?ïö{ô[ö»?G
Yð…ˆ"?S ŠD?G
Yð…ˆ"?ïd«¼Âú¢?›Hͪuè?"jˆlȳ?›Hͪuè?ïìîø	«>?pº ï1"M?c÷´™³?pº ï1"M?íô}'ŸKØ?'#Œ˜]½?°\lO{Â?'#Œ˜]½AGN4FGL J0529.1-2449c¿Èøч
•À<b›Zcù¥À:µ¡qÕ/rÀ<>ç;
H@‡0Á¾Ñ·@2ÙÏÏ?ńΆý‹¿£<§%Hcò?ÜjyMÉ·@Tgm˜Š?Ù©,߇¨¿çÑxÞc"9¿çÎ0_C\v¿ë]H~u|¿à@".þñ¿ïöÅ>cUNASNone?ïþöå'?
¸6Ýøœ? '«üM\7?
¸6Ýøœ?ïö±ê<"?VÄðâb)¦?Rœ,&¿©n?VÄðâb)¦?ïã¼mÐ?w
t?lçCÁ®à ?w
t?ïýeë[?ö¿Jv?4Ð¥1L·?ö¿Jv?ïÿ*SKè?!ÇEøÕbÌ?µš×;(e?!ÇEøÕbÌ?ïÛR$ÿ­?z]¢89Ô?rVí‹'ø­?z]¢89Ô?ïæΛƒÿ~?qÀ@"3y?i1du!I?qÀ@"3y?ïêi·˜vô?Y Ðöû?e–H%ŒÅ?Y Ðöû$AGN4FGL J0529.9-0224¿ÌiºÊFÀ32 D®…ºÀ:}å‰\4´À;Än@O{h@öE)B@>ñ³/m@ӝ_÷·?êt™=SH@²ß­*p@ÕD¬à¿ÑGËÂᑿÆ|ÊÌ¿êw½ü¥X¿ïW}_§/"?Ñ|#ý`='¿ÆNxÉjl°UNASNone?î÷-}´H?ºMô¦@Ø? (#ãô?ºMô¦@Ø?ï±NŸ¨ÚÞ?œ•þF¦ßQ?ƒ¬X"'à€?œ•þF¦ßQ?íOFO‰o?¤$«E"ˆ?µ‡ÝÎ͏?¤$«E"ˆ?ïëý¸ÇC?d3¶v®6ü?dGÂß%¦?d3¶v®6ü?Ép?¹Ž0ª5ÖÎ?¯÷WÅü³v?¹Ž0ª5ÖÎ?ëÓ$Ùdpÿ?ÊÇ÷ÐÜ{ì?À³lšn<?ÊÇ÷ÐÜ{ì?ê÷'힘?®JÉ'ÖҘ?Ä#`I…Ÿ?®JÉ'ÖҘ?ìä^cãA?ºæ©kñ?¸Ýàäù?ºæ©kñAGN4FGL J0530.0-6900e¿ï¶'ý6·À@:r2LƒfÀ7Öl9äþÀ;;¹ÿk@âQ—ø.Ð@ç±|å-í?¡š'_`D?•¦çÿ¶¸?öÛïqµ@±µ›ã÷?ìOu¹Nk¿Ô\Édb€(¿âµ†à‹P¿á×ÊÆbP¿á"€ãÀ.¿åpà<4dUNASNone3FGL J0524.5-6937LMC-30DorWest?ïïŸP£í—?[wEøÛ?``¯*˜	˜?[wEøÛ?ïßÏó6²³?Š©v÷Ò5Í?pm•¢D?Š©v÷Ò5Í?í/Ž£-?¥ h•¯?¶ƒAe%?¥ h•¯?îÄUÓNϤ?•;Eo?£º¢Ë¹?•;Eo?ï?ø#ÎÍi?"K§
?˜û‰•îÔ?"K§
?ï¶hê´‰?Û°ÆØ<?'eńi"»?Û°ÆØ<?íAÔá™8?¦4®Ëi|D?³ñYa)Â?¦4®Ëi|D?ë¨ßо&Ÿ?´
Ñ(?Á\€½eƒ?´
Ñ(AGN4FGL J0531.5-7823?Õw¬5ÓwÀ>…'¢xæÀ:½ÚgüÀ<J=k›Y@ÿW±Më@QÁ"³¦‹?À1{¸ˆD¿°z_þ©z?ðÀÔÜeÇ@õpKAœØ¿Á© ã9öœ¿åø þ¿ê'%ëbd¿ã Å®¿åAÝ¥¸?ŠñTŸC
UNASNone?ïþ¸_W~l?Ú§/?e?$ze¨¹8?Ú§/?e?ïõ¬õ–ðr?WDq[¦[¬?T¦d+œ¾?WDq[¦[¬?ïîa¡I€?_ëÃit?až^Á~ªs?_ëÃit?ïýßé¬xç?¿æüd‹?1´'²Ú‰?¿æüd‹?ïûèˆ{?F;™Yš½C?CÃéR'Aƒ?F;™Yš½C?ïÕ¬hd~–?|ù%n?u)ËÀ²1?|ù%n?ïÚbãҀ?{j¨´¤jä?rÎüŸô·­?{j¨´¤jä?ïæ¯0§	;?_Þ|bR5Ò?iPς2'?_Þ|bR5ÒAGN4FGL J0531.7+1241c¿êè:Hr¬èÀ&Ž·ˆ—é–À9Æ2Ôh£À;iÏûUvT@Š¿šàª@·V¾È'?ÐxR!5î?Öܒ½‡_…@ìÝÿ$7î?óᣖr¬?ǯ.–ÁM¿èrd×-©¿å—˜Ø©yá¿ë{Â)°¨¿ïû¤üۈ?éÛG¹ÒõUNASNone?ï1ì&·ØR?¹.͏«´B?™Â{*¼ÃË?¹.͏«´B?êxp§\û¯?ÄËì3‰3?Æ=bŒF?ÄËì3‰3?í«Ä9³Þr?>Yx‹?²¡Þ2aq?>Yx‹?Ꙋ~–?§¥RfR?řׂª?§¥RfR?îºèéãÞâ?¤ÿ{ÃY'?¤QqcyßÛ?¤ÿ{ÃY'?Êð)«'?Ì«4fòÓ?éCõ•:[¾?Ì«4fòÓ?ähÇw"vM?µ<ÙAÄã?×.q»g?µ<ÙAÄã?ÅgV›˜!t?³6ÜØU
›?ê¦*Y÷£?³6ÜØU
› MIXED4FGL J0531.8-6639e?ï?Ìw1÷À@K´¢3œÀ8ƒE§©ý•À;ŽÊw‡öÚ@ÚùªPv?ÿɌ;E‰?¡þ¾›B!?"‹|ÂÀ¦Æ?äˆô'
´@‡ÒFß8?¾
è¿×È¥`LEÿ¿áG
À²ã¿à+7GMœ¿â†òÍèU¿¿×Ôþ_
UNASNone3FGL J0525.2-6614LMC-North?ï÷zÇúß?mô?b*"l?QÃ
óûB2?mô?b*"l?ïðZ;hi~?m¸`»Íè(?_K‰"árz?m¸`»Íè(?îªïÇú?žJՍÑê?¥^×¢g?žJՍÑê?ï"v{ÿ¢/?€û)ç8«?Žâ`õÈ l?€û)ç8«?ïØaµŸ-?k(­˜\?sÏ%-Mc?k(­˜\?ïÓG§MP/?}ì·ÇÙ¨:?v\,H)ÜÀ?}ì·ÇÙ¨:?îúg\ŸW?š"cŸŒ¢»? _¹ŒÉ¿Œ?š"cŸŒ¢»?î±aP@Îì?›½áö Gî?¤éêû*B?›½áö GîAGN4FGL J0532.6+3358¿¹:;éyÒ?ÖâЯ°\TÀ9Õ¦k93þÀ;e·ÂyŒ´@Fj(ìç@'¼!ƒÞF?Îá\PãÈ?ÅФ®§?ö$SN[®?üÔ!s€¿à…°¾¤@¿æEMFÚ¯ä¿éùŒ|z¥¿ì}@"Ó¿ïÆa®pÁ3¿ïÿWƒuUNASNone?ïÃfÁþ?Œ:€"ë8?~>LU8ô?Œ:€"ë8?îýð+=U?¨8,ó!L
?  ýIÃø¦?¨8,ó!L
?âOYÉ?–MǛûí£?¥TñÛæJk?–MǛûí£?ï_¿êLv?ƒ›#Æÿdl?ŸôýP?ƒ›#Æÿdl?îà3jvҀ?£¨yÜ9ý'?¡üÉZJ¥ö?£¨yÜ9ý'?åÍg6x?ÑXå i}®?Ôe1õ'á?ÑXå i}®?鍲}½?³¦øO»Ú?ËÝÉ6Í
?³¦øO»Ú?åSTnu?¹dõ¬ðª?ÕÉ÷YW#?¹dõ¬ðªAGN4FGL J0533.6+5945?¼! Oðr@,UîþOü˜À:‹øÇ&›À<Y>Y#@"yq…ÿ3@I©¿Š¯?ÁczcHyÁ?äF]²b¾@©†b…0V@ÐÎí
Š¿æSø`îW?ʊˆD1³+¿àKý"z¤¿ëÑ q$0¿ïÿ®2D¡?Ô¶0=µm5UNASNone3FGL J0533.2+5944?Â+1Ò?Æ¿‹•8Ñ?ëu3»:Ëz?Æ¿‹•8Ñ?Ç_)Ší?ÀŽVšk{¤?ê;(5º]E?ÀŽVšk{¤?Ò®'^*Çn?²ÝW:å´C?樶ÐêœI?²ÝW:å´C?Ô"L=Я?´ÍPRÄA:?åîÙáw¨?´ÍPRÄA:?¿‰ïqVH?ѐgWcOl?ìÎÂÕ7?ѐgWcOl? —"ß½%?¤fþȺœÞ?îöÑöhŽ?¤fþȺœÞ?¨2vºŽ?ššZ¹Óك?î|ؗ˜¯?ššZ¹Óك?…¼zȇ¾‡?u†ì'5ä?辶çF?u†ì'5äPSR4FGL J0533.9+2838¿ïz)âҞÀ¤ì¦†çæÀ9@¹çíºƒÀ;!ÂÀ®@ƒvÐ@	ðÉS›‰?Æ*<Ó¿(ÆÚVM?Æè6 %#ü?ñ9"õjÑ¿á4PŸTÄ}¿åi¤ßGú¿ê#OÆðé¿ïúk _pÿ?í®/ªè¿ïÿ«±ÊUNASNone?ï¸!o"?¯…ŸRöYÿ?÷¤?NšN?¯…ŸRöYÿ?ï¸}	?•µè.Òü<?à½®Åzq?•µè.Òü<?íhCbw»Æ?£k+$|ÿ?´½äíÑ?£k+$|ÿ?ïû ¾b7??[Ԅ]µ?A}BŒ"??[Ԅ]µ?ï¯âvsi?•Ÿ¸\­t?"zíaåÊ?•Ÿ¸\­t?ìw1äîì?Çf@¾X,?¼Fp߈ˆ?Çf@¾X,?ìÑòÉ?¥ãéÞ{W?¹w/>¢v9?¥ãéÞ{W?ï"}öÐ×H?Ÿ©}'Qü¢?›°A,ÄNç?Ÿ©}'Qü¢AGN4FGL J0534.0+3746c¿xq\·Ü"@4òd/UÀ9£¶"|#gÀ;c¬sßÌ@þ©éèß@ϒ¯šŒß?Í7ÿuÁx0?¿Þ-G#*?õ{¡çEô×@	©f®ƒa¿à˜›ò9¿çò³ç#¿çCKK¶¿çùš‹1!
¿ïûdŸç¼g¿î<Ö 
L	UNASNone?ïü¼n…Ħ?3ÆC2a8?:‹ËAú?3ÆC2a8?ïä#õBY?wN%:–»®?kÜîC>y?wN%:–»®?ïǙN<›^?y£·´â?|3XåÑØß?y£·´â?ïî*ɓm—?H[½>}J?aÕ6K–)k?H[½>}J?ïüÿcšQ?9LAI
÷x?;x÷áÖ?9LAI
÷x?îî[¬'ßZ?¬-Y'Y?¡E5<b?¬-Y'Y?îúJCX?™Ašq^P¾? [V'~ôþ?™Ašq^P¾?ï…ä'U?zÃܛœ])?Ž†ÛgI";?zÃܛœ])(AGN4FGL J0534.2+2751¿ëÐ/@ÆèÀyž×ÆûÒÀ:e:V=#wÀ;ÚØä2D @"&H?"?þ
Ÿu{­ ?Äã׫M D?ŽyÁô?ʧÓC3†j@0a"šK?Ö©Ù‰s²¿ì+º~¯•?Åû…‡hêz¿â©4wž¿è
ŋë›?Ö¸qËõ6xUNASNone?ïü
´{R?2Y®¤álJ??'aw"žK?2Y®¤álJ?ïë6½Ï?p†9ey ?dpûÌáX?p†9ey ?ïÖgi+ù¿?wî1~V·è?tÌKdƒÀp?wî1~V·è?ï֖^?•0?b¼kÜÂ=?t´ÐÌG¬?b¼kÜÂ=?ïôž'6Yê?S	ˆ½Š?VÂÝÙKÐ?S	ˆ½Š?ýÊú?™ãŸ?Š'@Az&?™ãŸ?ïƒS0Ž¬?ŽòhɵC®?+3ó=?ŽòhɵC®?ïl»ì™Šš?ƒE@Ó¨¨?'h's­äº?ƒE@Ó¨¨AGN4FGL J0535.1-5422¿Í"ÿU$
•À@XÍJ¡À:V¶~¡ÇÀ<LtÎ6/@ÁV-ßi@qËa'Â?È;v8@Ž;?͈Šèü®<@]GóÐG?þvyÇQ¿åèÅP׉¿èaÊsc¿ãèS;wG¿ä«Àb±%¿ïÿŸóOîU¿ðUNASNone?ï«äj"]£?}Æ}]å³?…åzØ3>?}Æ}]å³?ï¥oz%#ë?Œç{Ì?ŽT?†¤!lh1b?Œç{Ì?ŽT?ïöå¥
ç?ÈÐý^?Á#F79+?ÈÐý^?ïÎëWsÒ?DÚ°$Gu?Ÿ""Y·Í?DÚ°$Gu?'K­º? »hN?¦gf×Ոk? »hN?í=ua´ƒˆ?¾ÕT©þ?¶Tñü¾?¾ÕT©þ?ê¡?«;®?­©±«éeO?Äõ{SJ?­©±«éeO?çÙì­½½æ?µ'5XÒT ?ÐL&¤""4?µ'5XÒT AGN4FGL J0535.3+0934?ê3oәçëÀ(@ÛH'ŠÀ:ìÏ¡"cÀ;•HFÀ®±@ÜѪF@¼mFTx'?Óœ"$'?ÝÝÒä>š@ko\¯-€@
kSù&r?Ñ{,܁ö¿ê5†öÿ¦¿Þ¤Cy|n¿ë¯
Ÿ$óÕ¿ïùu!j2ú¿ïüZžÜúlUNASNone?ïï2Rb£c?aŸMe?`Í­[d?aŸMe?ïé]XÃ?f
r;'9¨?f¢§}'Š?f
r;'9¨?íA¬{Q7´?¡-xǪÒ?µòœ%Nã?¡-xǪÒ?ï"ó›~Ý<?nNÓ£Yϓ?‹*—"÷?nNÓ£Yϓ?ïÌ[àüY­?{åYÌ}.B?yÒmåmy?{åYÌ}.B?𥳐˜w‰?ŒFáuWCS?…Yì‡1 ?ŒFáuWCS?ë»7;U–Š?©M0ù0Ó¾?Á#©¥Ö?©M0ù0Ó¾?íHJÕøUÎ?œrgد?µ½©Oaj"?œrgدAGN4FGL J0536.1-1205¿Öó;ÚTRpÀ6îיåÀ;\ÈWóÀ<†	g‡Î–@ K‹&5è?úV.u^Pî?֘"	\ ?å,Ýُ~@S1B˜+?üšÙ4ºð?ïÿë""i·?B;
ó?­x®ßÉK/¿Õ¬·¶Ì¿äTïE™¿ïþõU9UNASNone?ïòÎqƐ?WG$D–|–?ZcŸ½Þê?WG$D–|–?îÂZXº?«£ž©?£Ú^Æ4d?«£ž©?ï|Ò]Wô?…ڈª¼Š?e´W
—"?…ڈª¼Š?뻩I˜'÷?¡¡NWœŒ"?ÁZٝô%?¡¡NWœŒ"?ïî[^0É?`ì=4!Èb?a¤¢Ü?`ì=4!Èb?ë=ÌÄ
Ó»?Çñëx"j?ÃÌïÔ±?Çñëx"j?ï'‰?–U@¾ãµ?žÍÔf¡?–U@¾ãµ?䫨mzŠh?¼Ÿ:9Ú?Ö¨¯%
ë/?¼Ÿ:9ÚAGN4FGL J0537.5+0959?ë–^û|ÒRÀ&î™côÏÀ:#"D¾ÂÀ;œž%"ü@¥¾K°9@1·'¸¬"?ÊLå`íU®?Â*LDQ=µ?õ¸ÜÀ_×@"Äõ=l¿Ð]ó)®¿ÛëA,:¿î]©"â t¿Éíp†OåÆ¿åc¶ž78&¿ïÿöµšUNASNone3FGL J0537.0+0957?ïý€E#k?2axÐv¼?3ýÖ\G;½?2axÐv¼?ïô›L;Ô?Xwß⩪?VÉg—²Çe?Xwß⩪?ïš8·›Q?‡©/æ3?‰qÒmIï?‡©/æ3?ïûy`Ǟ˜?)=¼ö:÷å?B}‹{'?)=¼ö:÷å?ï÷±¤Ÿ©u?T|Éö¹œ?Pœ·G]ÄM?T|Éö¹œ?ïÓA÷Nß?€W³>ˆ?v_PQf!?€W³>ˆ?î/˜™"f)?¢ËYÁM£Þ?­viMRl?¢ËYÁM£Þ?ï׀",Ù0?h7$
ä4Á?t?îí4?h7$
ä4ÁAGN4FGL J0538.9+3549c¿ê7è ú@x7~òNgÀ9œ#…}ƒÀ;'<ðKW@\лnÖ@ ‰…O_º?Ê2(œ+o?ÕO´þÏÔ>@é>›A?ÿMðbF?北'·Ôî¿ä‡%"Ï8¿á&caNN˜¿ê^á6çÚ¿ëE¿&ñÜQ¿ïÿm²æUNASNone?Û6EÖgÄú?˸8¾ëì*?âdÝ̃?˸8¾ëì*?ÞreByø?˖öbX ç?àÆÍ^Ãö?˖öbX ç?è´Ij¤…þ?¯\êێX3?Í.ÚUmè?¯\êێX3?㌺¶ÓCè?«?˜G9C{?Ø抒Yx0?«?˜G9C{?Ã8&!§Å?ºo©
Þn?ë1öw– ?ºo©
Þn?­ìYz%?ºœì¹•ý?î!?Š{æÎ?ºœì¹•ý?ÇÂL´ACJ?²]2Y³>u?êlÒï¯.?²]2Y³>u?¯§Vÿ<Ìê?•IúÇrJ?Õ9r?•IúÇrJ$MIXED4FGL J0539.2-6333¿íÊn= IŒÀ@	d¾ÆyÌÀ;$Æ>=RÀ<Æ<üàÏ@<YC=A@0:û~'?Ë-‰ûìÊï?¬a´Mzª?âùaíÍÎ@zê,>¿ïþøÞ΂?ïØ#½Ÿ]S¿ë=nöWá¿´M"O£¿ä5o¸õs¿ïå`³IUNASNone?ïþQAï—0?CS~ñçR?*ëä5€+?CS~ñçR?ïõü‹i´?W'ÐzëÔ[?Tx‡Q ¸?W'ÐzëÔ[?ïã
mäl?iKçxä\$?lõ'÷¤j?iKçxä\$?ïúç"2û?,ºå§="¶?DcvÃÊ?,ºå§="¶?ïüj3¥t?=ñ⋷Zm?;­ò­íý?=ñ⋷Zm?ïÖ5÷]Å?~T•$]6 ?tåUìòå?~T•$]6 ?ïÑ%†>«?}KñYÄÎn?wm=Îf<?}KñYÄÎn?ïêbZÜ-?Z'"¾W÷?e¦'Rµ?Z'"¾W÷AGN4FGL J0540.0-7552¿Æ Æ4À>•#¯1±À:J ˆ5ÄÀ<Kìåq	@95:õIn@V—kÁïú?¿ƒ˜%{:?Ì#îX^¼@

òzœ@	N'î['οt—ˆŒî¿×9_\±Ü±¿ä/µš &¿çÂâh?"¿íÿ8$3»ï¿¨'õ:ªúUNASNone3FGL J0539.9-7553?ï܎I6š?mŠ×Z×~b?q¸ô=(#f?mŠ×Z×~b?ïñW}O°?\DAz€#?]Qr¯ñ²?\DAz€#?ï` ðŒ*×?Š(›:êÔ?"ëáîz¥?Š(›:êÔ?ïé2X¹Î?Këœ&¶³?fͧFå…?Këœ&¶³?ïré߂1?iÑG3Yï?'¢Ä]?iÑG3Yï?ïÁ]=¯?'¼bà¸?1Q"³¼a?'¼bà¸?ëbie/•Ö?¯Æ¸cBÌW?ÂvZkA¨¨?¯Æ¸cBÌW?ï^¾÷CE?€g–ck?"(!ý"[?€g–ckAGN4FGL J0540.2+0655¿ìÞÂÒŠÀ(Ü6q¬À:µ|8_ÂÞÀ<<3Ð$ë@!¼;ž½?ùcㄟ6'?׺àK}?ÍèþNe?úÔg–NÝ@[¹'ï?âˆö~vþd?ëȀB_¿âîà]Mc¿ÕmE	­¿ÈƒëÝ^?{¿äK™[†9UNASNone?ïý²OjmÔ?,'ýe¿?2m"Žܯ?,'ýe¿?ïóÂ+Dc?Zæ,}`Ê?YÞ{àpú†?Zæ,}`Ê?ïߟÅ$.U?s½[S¯rÓ?p0Š¡_?s½[S¯rÓ?ïó­Üû?CTõkl­?X¤ä³ÚP?CTõkl­?ïý["yæ?8#L˜E?5#Þ|FU?8#L˜E?ïÐœ4m_?€½¾F/y?wù±õ—"‰?€½¾F/y?ïʧ˜'9Î?ä)haÆÍ?z¬3ÍQtï?ä)haÆÍ?ïÖ2N†Ë·?j°ܳ ‰?tæ؝­¨Ú?j°ܳ ‰AGN4FGL J0540.6+5540?裗y%RA@)ægrÕàrÀ;u"ÁËèÀ<VòQÁ"´@s"à?@¥vjNR?Î7'^"´'?½¦ù>ì?ðÿfèle"@@o7›LÍ?íc\%šÄ<¿ÕgnÙ÷¿çùƒCì¾Û¿ç¡Ó#þâÊ¿Ý5ý''¿ïÿÿ)@k*UNASNone?ïþèö¤¸?§àÍx?!p•il«?§àÍx?ïïøpc?b*8ÙÙ?`ï5I_?b*8ÙÙ?ïí/Ý«Ü?[´L¡6ýˆ?bÐéU.[¹?[´L¡6ýˆ?ï÷_ÜÎ;|?5ÔÍۖBe?Q@FÀþhH?5ÔÍۖBe?ïÿ1z½p?ìêÁ˜­%?ÐÄšã?ìêÁ˜­%?ï¨$"^ò)?]6¨7àû?…öÚèCuÌ?]6¨7àû?ïݶ£"mÒ?uÜñçfì?q$®,¯?uÜñçfì?ïÄ>}#
?në¬Ok……?}àÁmÀo>?në¬Ok……AGN4FGL J0540.7+3611c¿ìFz
»£b@}úâ~À:Ç=@Ó/À;dS‹'@'Œ`÷@‰3¿Â?Ðǎß×@™?àtüÌnØü@4zøÄ¢?ù¢îA'šÈ¿ï÷"}~[?ïÏü'$y¿á9NÖ&é¿ì3шô/è¿ïñò¡ų?îÞëuUNASNone?ï(jØ;?£v«êëK?Ÿ¼ú÷Ìb–?£v«êëK?àåµí?ç?͙À®¹ïÙ?Þ4"%€1?͙À®¹ïÙ?ê ü®€ =?©Ô˜Ñ¦.?Ç|
Eý?©Ô˜Ñ¦.?ä¡{P`ô?´šã…EÜ?Ö½	_>×?´šã…EÜ?ãš]•Ìk?Ê°!gÑ?ØËDÔgÃ*?Ê°!gÑ?«r09§Ã2?¸â`fTð3?îHÜü­?¸â`fTð3?×r3N6ì?¹'eow?äFæXäóŠ?¹'eow?ªüÊI~ª?œRårc‰b?îP3[nˆ?œRårc‰b0MIXED4FGL J0543.5-8741?ÙgT®—
À;ÈCރÀ:ÿƒ~`À<h30®ôu@M²³ñ߁?ÿžÔ¼…Vì?Úp™›&?ÁD°E­‰?üg+ˆD@×®7`iw¿ã}ú»×\¿ép|4.ö¿ß5ßJ}Ҕ¿Ø~ÿlÅ¿è9¿¾ëc¿ìA\[ðlUNASNone3FGL J0542.2-8737?ïûðÜÿþ[?9Âõ"?@<‹ÇóZU?9Âõ"?ïó[Ã[p$?YÛ©E…?YHy¬vª?YÛ©E…?ïê–϶?j«J=0M(?eûj1ˆ¡l?j«J=0M(?ïè=MŠÄ·?PƒÐ	%?g²n\?PƒÐ	%?ïĐè'r€?ƒ¢
Ýh?}·‹´¶ûß?ƒ¢
Ýh?ïÒÉqߧ?}ó¸Ë˜W@?v›G^†?}ó¸Ë˜W@?ïh‡¶BFÌ?"øÂÛ¤s?'ï	<ސk?"øÂÛ¤s?ï›+ç±Ìä?x3î.ÈE¤?‰5$ºÓ?x3î.ÈE¤AGN4FGL J0543.9-0418¿»ÆóL›íÀ0ú;%oüÀ:¬	æ~À;©Jß!c@¼Òo£üÊ@‰4\(?Ì
¾±:u?È·~Fï"@%cµ±þ@à™+µp?ï¿/À·ë"¿Ù­ÜÊ5ï¿éŒÏƒ³~¿ædËÇOh¿ïÿò"²¢?ïÿ9fS0UNASNone?ï½+Rß7?{O†™˜]&?€µ+qy<?{O†™˜]&?ᅳ"Oä«?‹±òÊÆú?€[0~S<?‹±òÊÆú?ïCêÝÑN?æÒƒWå?œ—' Ö:9?æÒƒWå?ï}_gÕ¸j?tóm^sñô?T'$Ã?tóm^sñô?í6ðYL€?´Ê¿#Ý?¶O~íiý?´Ê¿#Ý?íTé2Öcq?¾ˆˆòyÒ?µX¶j(Ëx?¾ˆˆòyÒ?莈/8'?´ù•%‡?ÍÅßCƒ½?´ù•%‡?éqÝÞ"?²(1T¾É?Ê8ˆ‡£wê?²(1T¾ÉAGN4FGL J0544.4+2238¿ïÇZÄ¿®À3F~i'À:YËUÔGëÀ;ˆöšüp)@ )¡n@Ø
±?ÄóÈd2Y™¿±{PƒP,?ê+Xx`å?þ(V˜½üz¿ëþ¢1ìÞÎ*L…¿âÐÞßôǾ¿äXxœÉÏ¿éÔç¸á]~¿Ð³HAbJùUNASNone3FGL J0544.7+2239?ïðw?UX?Y'}•Lmð?_ÛØp~?Y'}•Lmð?ïÚê µ5?oƚ³g?rŠðu$'n?oƚ³g?ï{Ao¿‰ ?Š.A¶–-?—Ò	Æ©ý?Š.A¶–-?ïԋ:0Rƒ?aù^­Ö?uºbÑÙ>‡?aù^­Ö?ï,~èà¡?™Æ¥Q¤1?šp"ì'äe?™Æ¥Q¤1?îËrn©Î=?±)]š;µ?£HÙ‡59?±)]š;µ?î3šwÂ? '<±9³?¬Ï¶XŽƒÞ? '<±9³?í¦Ï°?¥-Ú]øçZ?²É'}ÑŎ?¥-Ú]øçZAGN4FGL J0544.8+5209c¿í‹hG"d•@''éÌ·ÔÀ:´4osUbÀ< ÇË)_@<Ä~¾Ý@õŠžT~?Ȥ֎—ˆ?¡ä´Âa[\?Ò6§|0R-@9ÌÕh¿á_ç@ìYZ¿â«Ûmi¿æ/Pà˜0¹¿ëù=í¡Y¿ïiОh‹Z?íÚ¤ü¤*íUNASNone?ïûVOÂàæ??P¿@®zV?B¦ÀØÿ‰X??P¿@®zV?ïì"*ÕÊ*?iñW–ôí?cÝÔúN5?iñW–ôí?ハ¾¾ƒ?u?<C?€]PˆÆ?u?<C?ïñȽ/v?HÂóªY?\oÂd¤Ôe?HÂóªY?ï÷€#?¹î?MÖKê¤Ð
?Pÿ¹ù~c5?MÖKê¤Ð
?ïi''Ÿ
?¡åt{x¿?'ÛŠ"´Í?¡åt{x¿?ïhMœÉ's?8a]w†H?'öLc`¢?8a]w†H?ï]~òé?‡Oažä|?"P!«veã?‡Oažä|(AGN4FGL J0545.7+6016¿Ç;ÝÜi¢Ü@/yb(D€À9Êãv\}¯À<P•V=ú7@Hñk<¹ð?ýHÅ¡_`¹?µ–…=5÷?ӋÄY`Äf@çíA·Zu@Ç=˜^?ïïÑ|^ö¿À4âµÂD3¿Èô±ë±¿à¡'A5ª\¿ç«
Û%U$¿ïúo!ËׯUNASNone3FGL J0545.6+6019?¹Ò"ˆ^?ÀfËÈã*ª?ìÅ®Žô?ÀfËÈã*ª?Ê;üTÀ'?Â*!´Û"?éqêûOÜ?Â*!´Û"?Û¾¼Š±Ã?µpŽc¸¸?â ¡ºò§?µpŽc¸¸?ÓdLñgy?±X£»0·?æMهpLC?±X£»0·?­e"©P×ð?ªOä°3?î)¦Å¯ª±?ªOä°3?¥Óñø?¦Ø?ç"[?î§âÆøç!?¦Ø?ç"[?ݕ¹i‡qé?·*µÉ¬;?á5#K<G?·*µÉ¬;?œnþ,ĘÇ?‰«æ7o?X?‰«æ7oPSR4FGL J0545.8-0905?ïÃ4ô»À2­«ÀãŠ~À9Ó
ÙwÕúÀ;‰ùºk¡9@¥Þ^sS@Ð$ ?Àô+uúƒ?¡Ÿbûþ?ãÒácÝ @«ð¥oØ¿à~‹ì¿æõÊÝ^jo¿á>Nàð~¿äx6½¬Hs¿ã߃VR¿âñ+Pæ¢aUNASNone?ïû.ûH¾¾?:ŵ駝?CDžˆŸf?:ŵ駝?ïõ'ø¯m…?U$Âð¢.?TÚ-²E?U$Âð¢.?ïê†r0°2?g–e²äOÀ?eyÁ']Ë?g–e²äOÀ?ïòœS¢c?Bv4
›;?ZÇXtƒ[$?Bv4
›;?ïçjÂìy:?d†nÏ*?h•<Õ­Í×?d†nÏ*?ïØ(س­?|–ÉÄ{bÖ?sôë¦ãùI?|–ÉÄ{bÖ?ï±'Øa*'?†VÔ²{;*?ƒ¶	Øï	?†VÔ²{;*?ï±
ÚfÆç?sì¦Ifäƒ?ƒ¼‰\¯^J?sì¦IfäƒAGN4FGL J0546.5-1100¿ÜÎÿ"À3U¢Æi}À:a՟Ú%{À;Þ|2€…Ì@'Áºõà@"ÕN´™?Ñh·#˜5–?âý ⣣´@|FØ+¥ ?øwÛ¿ÙþŽÑ¿{¿¸Ù"ì
"οêEœVã;¤¿ì­Z˜¿áðk¢æIv¿ïùOýnUHUNASNone?ïuF°~Ê?¯Êù¿ÈM#?'W*‡ô¾?¯Êù¿ÈM#?í
oõRÊJ?¸ÀžÎqC?·¬€V³ˆ1?¸ÀžÎqC?í²6X#$?7},Áù?²nM>æßa?7},Áù?팟•ºš?—5Ñ6#?³ŸûvD-?—5Ñ6#?ìí°ãjю?º"n5¬y	?¸'xä©s"?º"n5¬y	?×之…w?Ð%Wó†õÓ?ä
£:=yÄ?Ð%Wó†õÓ?çFšZM˜(?³z±…^f?ÑrËKdÏ°?³z±…^f?ڛ<Vp"?¾õÞéÚϚ?â²aÔ±G¶?¾õÞéÚϚMIXED4FGL J0548.6+1200?ï']ªô$À -i ­ŠÀ:3v†ojÀ;¿·lé7g@5XûC؝@³Ão1?ÏÚué‰?Ç6%ö4?ëÆxõµ#c@ú¨ïLÿb¿àóÛ>ªŠ®¿×ëD‡•¿êV¡'M¹¿éûibš)¿ï²Ô2ò›"?ÛǚþôgFUNASNone?ïèrÀF×?k:°Ü~?gî±¨%?k:°Ü~?ïíä`"µ?iNÆQՀ?bŸå®[ ?iNÆQՀ?ïF]µ<ã?‰•6G4¨ñ?—=TD0ù ?‰•6G4¨ñ?ïéüôeu®?P-wCT…?f·g	¢?P-wCT…?ïlàsÑ;¥?•­Ácâþ?'cñ…Ø‹a?•­Ácâþ?¶Ó2º?•8C/®,?ŠšÒXñÁu?•8C/®,?껺Ž0Ú¾?°¬Rg±õ?ÅÇ<•?°¬Rg±õ?ïف!cä?ŒMW1ü7°?œÄÏâ²»t?ŒMW1ü7°AGN4FGL J0550.5-4356?áÏê>€KóÀ<ÿ‹&9O­À:¯ËlÂÀ<™TÑél@@ }7Š…Õm?øàYÜë(?ÓOÎ>¼Ô1?Ïsû$y&?õÀ›€úfc@}hLðô¿é«ç¿ç4=õ.¿æ=•W¹Ë¿Â…"¿µî¿â·{ây‡U¿äkg†ø­UNASNone1FGL J0550.8-4400?ïü¡8èl?1˜ÉvQ{?:ö=5ùâ´?1˜ÉvQ{?ïõWLr?U–¦bêi?UQfjé;?U–¦bêi?ïßèåK³?c	#°­^'?p_ù¶?c	#°­^'?ïòÀj¤õ©?AÁŠ¨>?Z+‹L¡?AÁŠ¨>?ïý"æɚ‹?-˜jûÓ?3`ÊjÉü÷?-˜jûÓ?ïÖ¦
ôj?|DW'™?t¬ùäc(?|DW'™?ïÖ°=ƒG?x!É1}™?t§áYñhÜ?x!É1}™?ïÎt<gåB?j]­)?xÅá«Áf?j]­)AGN4FGL J0551.7+0446?é"e˜¾±À%î°t§qÉÀ9±*˜YþyÀ;…ùTTK@{"úX¡@4"Dž?ËO'ŠÝ>?á Þ'ö @w"}Š@£tvŸn›¿Á¯…,пÝ;%û'2¿ëC–ß~*¿êï/}œ
¿ð?ïÿÝe¡D‰UNASNone1FGL J0551.6+0449c?èH"×V¥?Æåòí%?Îߓt¢¥m?Æåòí%?é¹h¼ûî?ÆÌ᜴ùi?É]
øG?ÆÌ᜴ùi?éÀŒ'u
?«Ø°ç±-?ÈýͶ+ˋ?«Ø°ç±-?ë~9ìµËS?¥Àx|	â?ÂM(Ò²?¥Àx|	â?ښv‹¦?͝¥2æˆ?â²Äºsr­?͝¥2æˆ?Äe^zDûÄ?ÇîW6È?êæ¨anÁ?ÇîW6È?Üõ˜×ì^?ºÜgŒ<?á…3"	ÀQ?ºÜgŒ<?Ãa7CtZ+?²9V«xãB?ë'²/"éu?²9V«xãBMIXED4FGL J0551.8-2130?îUþ
ÇÀ6Yl6KìÀ;jlËÛ5EÀ<°IpŒZ@%8ZåS×@1¡šïÛ?Ñÿƒ
6?Ëàs±B?ö"ÐÜüÆ@â×P3t?î3Îc¥ÁÆ?îšcX"쌿àMªx.—¿êå"Ï7á¿È/ïÜÇ@Ç¿ïÿ~À¥L*UNASNone?ïô'žÐD?pí©rFòÂ?VÜÃþݗ&?pí©rFòÂ?ïñ4¢ÁWñ?agwø#¥?]–ºó'­h?agwø#¥?ï®
žƒR?'"K©¦þ?"}XléèZ?'"K©¦þ?ïð"©ðvB?KjëXßÂ?_º¬K|‰?KjëXßÂ?ïéº?›:G?m˜`
aÞ?fEÀ"Í8ó?m˜`
aÞ?ïÄD¬=œT?ŠCƒxËå?}Ý©êнû?ŠCƒxËå?î²TæX±i?›YØÀIQp?¤Ú±žÀld?›YØÀIQp?Æz^?€€$Q'Ê–?‰?Ÿ'Ñ\?€€$Q'Ê–AGN4FGL J0552.0+2656c?ï––/ô?Çh'œ&;ÔÀ9—ž™ À;8ûefŒ&@›Ñ,Wø@[œ›¬™Q?Îb~ºÆ?Ú	{>d¿?ø¬Gõb?ò?߉=¿ØAN^²½Ø¿ß1BªŸ{¿çeQÉ oâ¿èÊ/cšÚ¿ï.mÚÚ¿ï;^g"dUNASNone?ï1œ@y(?³¬—WõàA?™Ìt??³¬—WõàA?í.K1N#?¼±{fícµ?¶¦si%«?¼±{fícµ?ìk׋äò€?¤
Ý«K°ž?¼¡C Øl?¤
Ý«K°ž?ìaOJô? €¹Yð´?¼÷ý…¯àa? €¹Yð´?íjhZ9î?³(>w.ìš?´¬¿äV?³(>w.ìš?Ýd"0E\?Ó#˜•&‡?áMöîçÝR?Ó#˜•&‡?ä|NxÅê?¶k¢I…Hî?×cuÂ-?¶k¢I…Hî?à*cbÈCž?»t-ÏF#Ñ?ß«9:oxÅ?»t-ÏF#Ñ(MIXED4FGL J0553.5+4810?è8ðòúf—@&HƒýP"À:—Ò+ìîÀ<¾mŽxÔ@Ö!·4à@O–áXu?ǁð/¨d?FÚ
Û¢¾á?ÿ	"=—¿å Ã6iI¿æ@š>Û"¿ì¿†]|²Ù¿Î£¼ÞLù¿ïÿýF\I?ïÿÃÏÎ	
UNASNone?ïÞ䢛[?q0GZ,}T?p¯rI?q0GZ,}T?ïë)ÆÅC8?o¨ÃTgY*?dÖ9
að9?o¨ÃTgY*?ïb-¸ÍÅ?¤Ä?ìq[?"ºN
±Z?¤Ä?ìq[?ï÷Õö›þ?@OΟì"÷?PUÎ/^],?@OΟì"÷?ïµ'_ž?‡¹¸aʏ?'¸›qpê©?‡¹¸aʏ?ïZqâµ0=?¥Ç6¿<'ï?"±Ã¥ê\k?¥Ç6¿<'ï?ï'¥—9ÿ?"w¦…¹‰?›M)ü?"w¦…¹‰?ïŽ;ËæÛ?ƒœ†=±8_?Œq
5',?ƒœ†=±8_AGN4FGL J0553.6+0100¿Ü ìr?‡À(¸mµ@æÀ:jíLŸÀ;¶3PdŒ@'Ù®¸»@ß	zÓõ?Ø^K¥Dóz?êCXz™@H¼¾aÏÿ?ý‡¼!ƒÞ¿Ð¯9¾èˆ•¿Ú"ã"Ê*¿è0‡‡H^>¿ï¼sÿP³?äJ
M{¿ïöÿ<
ÈUNASNone?í~ð±–Þ?¸Ò …ÍÞ?´zwb?¸Ò …ÍÞ?ìC떀N^?žx¯êu?½à£Ký?žx¯êu?ëjXR@X?©¨5Ĭ­?ÎVž¶þž?©¨5Ĭ­?ïohˆÅƒ?Œ¾=D?'ýt¹?Œ¾=D?éY;¡¹?ÇúöS·jÃ?ʛ‡y—?ÇúöS·jÃ?ÐщNa¦¨?ÐN½Ÿª¢?ç—;XÏ,¬?ÐN½Ÿª¢?á}	ŸªÄ~?¿T&^(L?ÝìÀªw?¿T&^(L?âGƒönÃ?Ð}Çô?Ûpùæ"z?Ð}ÇôMIXED4FGL J0553.9-5048?ê-ý¾©•ÝÀ=ˆ2¹¯æÀ:æ9ïôÀ<³ªÉlÆ@s*ÈU™º@«`¼z.?Ë{O+·=ï?¹o0'ˆ?í
Ž>F·Ÿ@S—ÖJúпä¼ò.†%I¿ã—¢^S*¿æ»ÀÖ…&¿Âf%cf×¥¿î
?¿2°V¿ï' 
UNASNone?ïûÄ= ?RF	čڽ?AÈî¼U¡ö?RF	čڽ?ïõûO=¯?Uå~ØvÆÕ?T	bO6':?Uå~ØvÆÕ?ï×ÊЯk¤?qébÎAd?t—¸aØ?qébÎAd?ïöYÃ?Û?;†q+Ý?SÍM0øÖ?;†q+Ý?ïý}†_ø[?+jË©´oö?4Î鶶?+jË©´oö?ïÙ·Íø
?{ks
¢'?s$‡áñW?{ks
¢'?ïâ‹U盹?x2‡.
"þ?mtª¤—N?x2‡.
"þ?ïÖfU¹4?fRØ¶Ó¥?tþLí0©ó?fRØ¶Ó¥AGN4FGL J0554.0-0839?éÁ¦y¦àÀ0§õƒ¥À:yB¾ÁqOÀ;ú¬ûv-"@€ÝŒb¤e@ÿñQçSa?ÊÒ¥û|¹?À–Dû\­*?ôGòø°€f?ø>3i¹×þ?ïÿ*bT3¿ÝhLðô¿ãÊGÅwÄ¿âÅaôfſ揉	ÿ]C¿ïòd6
~UNASNone?ï÷ßýxˆŸ?Y@ZwÀŒë?P@^ô@?Y@ZwÀŒë?ï¬Qˆ¡?Š–Xù>»j?"ë¾× Ì?Š–Xù>»j?ïÂÝt(µ›?~š5m™I?~'EÎŽÜ?~š5m™I?ï'œòP?zGf¤'^r?Ÿí®La¶?zGf¤'^r?ïê0ÓJj?gQ´•­Ù?eÏãù¥Õ?gQ´•­Ù?îauQvüG?°þCâ‡?©èªêH	Ž?°þCâ‡?ïQ©u§?™ؐ$zß?ŸÕÊà)+?™ؐ$zß?éKPíb?§áÈucÕ?Ë¢Ò¿øJv?§áÈucÕAGN4FGL J0554.2-0259¿¼BñŸÈÀ,'gn¤"ŠÀ:>zt:d€À;¾G^cb¦@%ï6¯©@ys{øžã?Ám6åtÆ¿ŒÃëk0™?ÌGԪ矷?þN9Vé?É@ˆÆ¸‹¢¿àqöó4¿í¦ÉB~ª«¿âê®ñ𿑶N[,Ìg¿ãêJŒL˜UNASNone?ïø(ÂZǼ?F†Ø²uÊ?O\÷Qq.?F†Ø²uÊ?ïóÉ>*«?X>@"ãÕ¬?Xmƒ‡"ºe?X>@"ãÕ¬?ï® møoØ?í©ÿßÉ?"wäyM&?í©ÿßÉ?ïû€£ö·#?-yØö5e?Aýp"½(9?-yØö5e?ï¯*g²–Á?ÞÐ#$7?"5fÂ	Ô?ÞÐ#$7?ïÎK:n™n?€&R¾(›0?xÚb¿`á?€&R¾(›0?ï˜Ukú?"Žc%V`;?žìõVñ¸Æ?"Žc%V`;?ï̞äñ\?q?ÕIã?y°ýxÎ+?q?ÕIãAGN4FGL J0555.1+0150c¿ë…h´
RÀ'GLnm›åÀ:F¹"À;£)¼'ì&@úîãøãV@ŒT6¸ú?ÎÕ1J?á@B,Ja@Çþ0òç?øÇøâªY°¿ëL§ãß8	?ï·C[Ÿc¿à;Vƒš¿ê=sº¿ïÿýç!é¿ê]"°§UNASNone?揠'&ûº?ʦ—óàY?Òà¾Ý²Œ?ʦ—óàY?ÕæAHÛÍ,?ʕý;ï3C?åß['j?ʕý;ï3C?ãƒÜ^n?²»¯1"¨?ØùÛØGC$?²»¯1"¨?Õu•äzé?¬Èɕ²D»?åE5|
‹?¬Èɕ²D»?ÃÿMóÓÍ?ÄÑI<	?ë8lƒ
?ÄÑI<	?²Íl;qØü?¸ƒ8â¨3ï?í¦Rx"q?¸ƒ8â¨3ï?»†x!P
?¦$‹ÈȽ?ì0ûܕÿ?¦$‹ÈȽ?' ÊfEMJ?{ }'Á§ï?ïvù¬²X¶?{ }'Á§ï MIXED4FGL J0557.5-4452?îS¼k3]XÀ;óìþ›{òÀ:g%¹Íì‡À<NØúØ@êç§Ä¡@t¹­6?ÂSÕÀ{ο Ş°.Ü?׍ÀÿA@špkø̅¿×@>^Šyì¿é2"²¡¨¿êÈx	&o¿â¾N"ÈQ¿ïþ
·x§²¿¶²$ÀS UNASNone?ïý{͚–Þ?3ÿÞ¤êöN?4!'Ò	è?3ÿÞ¤êöN?ïõ•lI~?e÷lçÎH?TÕ'Qb$6?e÷lçÎH?ïáõ®žA?i¹ªYÒþ™?n
ú$ç?i¹ªYÒþ™?ïü ]©ºŠ?,«èfï¢?>ýŽÌÏ»?,«èfï¢?ïüjµ¼¡?@¯$ƒ!u?<ªRÔȎÿ?@¯$ƒ!u?ï×krÈR?}"c'ù?t~ÊY)ºØ?}"c'ù?ïݓŒk©?xˇ&¤ø?q69ú*±?xˇ&¤ø?ï×êòŸÉ?i,:é†|?t
†¤Èïl?i,:é†|AGN4FGL J0558.1-2113?éþ"_4À4à¤ãy·|À:USʂo±À<jT¨ÎÀÃ@¿(Y@ˆœ|&Â?Ǩˆòß[?Ѓ­Ÿ
ã@÷9zu$?ýs$ºÊl?ìO"¢—D*¿ÆjOv`¿å—ö+jçտݗ|ÞÍÖ7¿ífNžHªê¿ïÿߞ¶ŽóUNASNone?ï—ËTÁg-?'7K0)o?Š
*ÅW`Û?'7K0)o?ïZ¬©–¼Å?"´.XH"?"ªjÆI/\?"´.XH"?ï
0ïÐÌ¥?'R«äîÙF?ž¹â}qE?'R«äîÙF?íɉ;Þ?ŽUY£µQ[?±³·ÖZ:?ŽUY£µQ[?îFü#ºð?¤,ŽU".D?«?zTµ?¤,ŽU".D?ë÷(pa'ë?Ào-AN l?À#^>y¸S?Ào-AN l?ë'>¿·Ô?¬çÛΠÌ?Ãc± °?¬çÛΠÌ?åŽI'Ã?°ãas>d_?ÔãmÌûàz?°ãas>d_AGN4FGL J0558.2+0132c¿Ø%­ÚÕ_TÀ&/¢ß"xîÀ:?ûUvTÀ;¨
^u×@žÒmö} @ÉzUý?Ôæ‰ah$×?ڄKßQ‰µ@
;3Úøßz?ÿ†xÕ~Í?íµ"Ód—¿ßƒf|`΢¿ç•jËOõ¿éŽ•¹:I¿ïÿÿ>¹ú?ïc!u´UNASNone?ï€Ñ¼u¼›?Žºõ¶8?ËæuR?Žºõ¶8?ìAcÚMœ?À$­ÎɃ?½÷¼á-"?À$­ÎɃ?íKŽÍs÷Û? ÔQ8r[i?µ£‰"`A+? ÔQ8r[i?ì¹úÜñ÷?Ÿp˜¦-?º0)€pJ?Ÿp˜¦-?î4A-Fà?±@»êñ?¬¿»ê—Ý?±@»êñ?Ñõ^çAL?Ðàƈ‰?çPŒ_tZ?Ðàƈ‰?â'¥šó{?¸*ùÕxÖ?Û±ö´Ê?¸*ùÕxÖ?ÏGZ¿`Ÿõ?·E®rà?è.)P'Ø?·E®rà1MIXED4FGL J0559.3+0352¿æùõ±˜À#"Š½]ÄÀ:	-ãÀ;±6½+o@µðöøš[@-¾Ý '?ÕE~ð ç?ïÿ› 'V‡@è+}\L1@¸PW†N¹?ï[Û]‰H¿¹C`Á¥–¿îFÄ	¯¬+¿ìÇæîð
¿ïٓLØ ¿èñ$?¥\pUNASNone?ä˜IPkd?ы'Í·P?ÖÏmß_)9?ы'Í·P?æ߂qj«?É)¤FÏOç?Ò@ûÿ*©?É)¤FÏOç?éÿEðœ'?­ð/°û>?ÈÊè=÷?­ð/°û>?â¦,˜%?³—¤FÒ¿ƒ?Ú³¦ÏÑÓ·?³—¤FÒ¿ƒ?ٙkS§?Ðå:'K?ã3JV,u?Ðå:'K?È0á¹á
?ËsPôSe?éóǑ¾G¾?ËsPôSe?ދjÏ#5²?¼Œ^)£^â?àºJ˜ne'?¼Œ^)£^â?°$²Œ»­?™ß%k©¯,?íüi'ë«?™ß%k©¯,MIXED4FGL J0600.4+4949?ïÃؐ@)ž™Ç¼Â"À:í¶ÓfDÀ<Jž6·L@ _Ž…ê:@´Å¤º_?È{T44ºó?¥S°ß¹ìÿ?Þ–¼f@Lyð'οë(øçÝÊK?ì*³Éƈ¿î\.Õ?ÆÐ{k0P¿é"3É[(E¿Þ¦ž9çWUNASNone?ïñ¥Õ|?":\³X?\µÙSãhÛ?":\³X?ïꠂl"?j‡¸Š\"?e_}Š`"Ù?j‡¸Š\"?ï¯Ð4,Ϲ?Žç°D(?"òîDϼ?Žç°D(?ïð|äÏoa?EéKìsA?_6‡œÞ?EéKìsA?ï‹È¸7‹Õ?Ž™`cÂó?
ÒK²?Ž™`cÂó?•êý(?ž†žcY î?Vš‰Þ?ž†žcY î?ïAPrÔ*?'9RËç?—Õü.5Þ¹?'9RËç?¹q?ƒcãîì >?}ßzS¢?ƒcãîì >AGN4FGL J0601.0-1016c¿ïN<»"ŽÀ/žj±NÂÀ:XÌ'©»À;žøÐ`Ö@¡di6$@
X³ö<2?ÏÇó^±ç?Ü®W+`@ü¼Ï(ǟ@Ñõ!T¹k¿Æ°(|Jÿ-¿ØiP{˜|¹¿æ£mùÞý¿ëá¬Bh°C¿ï÷íA·Zu¿éˆ²r®sUNASNone?ïÕØVñ?p
Ïóc©?uÔ·"Ž½?p
Ïóc©?ïª\öX¿è?ˆ·˜½c"Ç?…hÂ\–?ˆ·˜½c"Ç?î[ʳË}?–è•©jµ?ªOóSça7?–è•©jµ?ïQÒULãˆ?uÈ`±'?•ÅµRóòõ?uÈ`±'?ï2fy܏ã?–læ†}?™³0Än"?–læ†}?í0ôARR?ºn"SGŒ?¶{^ÑTn?ºn"SGŒ?çÒŌ^*?´"ß²úàÿ?ÐZtçC׬?´"ß²úàÿ?éÄ!qâû?®¡·_Ó$U?Èïz8w¸?®¡·_Ó$U!AGN4FGL J0601.4-6057?ï1GhIj'À=|MüãÀ:ò{+‰>À<'é]ýY@¼úh;~@VÁBU&?ÓBýwºw?ÒK!{û£û?þZ%zãËí@¥Šeôül?ﱚa•œ4¿èHâA©¼¿ãtŸM ¿áà1~'ML¿ïÒŠÝ>4?êpYddIUNASNone?ïêÁÚ!ì[?\®o•íC6?e>&m<]?\®o•íC6?ïè[Ë=?oh8υˆó?g¤è9Kl?oh8υˆó?ïQ¿$îvì?ˆÌϯˆÌË?•ÈgXŒ†?ˆÌϯˆÌË?ï҂ئ¹'?^غcåó?v¾""•û_?^غcåó?ïæ-"åÅ?kÔ5nó8?iÒݽŸÛ?kÔ5nó8?¼×·7?'¦MöǶÒ?ŠÃ2úf?'¦MöǶÒ?îQ•á©(?œõ ï\ñR?ªïÆ¢ÁT?œõ ï\ñR?ôÅdN?".‰	¼\á?¥µ ´…¢$?".‰	¼\áAGN4FGL J0607.9-1904?ëK èá^À1쇇H^>À;-ÕctCŸÀ<Û®ïl@ b¸¬.q­?ÿ{ ÒÞ^Æ?Òâðe-VO?¾æÒ1›Ä?êÔë´ï`v@l´S"6†?ç¤ÂAÉy¿ídƒ¢·O¿â8j_oQG¿×Õ'¤´ªÂ¿ÝpĎ9ê¿ïÿ'þKÊÚUNASNone?ïý·âô›7?'Hâ$¼û>?2@é;s/#?'Hâ$¼û>?ïôLP™(8?VÍ7R¿üî?Wg^¯rÿ¾?VÍ7R¿üî?ïî³=ïŒ?dÆagêÆ?aLÃ/È£%?dÆagêÆ?ïôs1¦§?:G)¹O«?WÕAýÉ?:G)¹O«?ïý§ÿŸE?0íBù¥Ï?2Àغ"?0íBù¥Ï?ïÔÀECÅÁ?}üoÉì?uŸÝcœL?}üoÉì?ïí;ʱiš?nˆp§¯?bÄ5c4
ì?nˆp§¯?ïŋswW6?lGlxhº[?}:F7õÍ;?lGlxhº[AGN4FGL J0608.6-2305¿î£÷ŸšuÉÀ3SÐÚèÀ;LÂPrÀ<ˆœC˜E@ápÌÚ@‰ë têŽ?ыÝÄ@â?ÕHK=–
ž@¦±\.?ôV¥‹•Iÿ¿è8Eáá†î?ÌùÁâãåm¿ç=|'‡"C¿ÞùŞ…;¿¿ïÿÌ3IÙh?ïü,d1UNASNone3FGL J0608.2-2306?ïÐ÷ìƒ?tkœÀœf?wúï¾z?tkœÀœf?ïgN˜¿T?¥Sza¬(¤?œ3.Ÿã{?¥Sza¬(¤?îl¬6\æé?˜e"Ç.æ?©5<–Áõo?˜e"Ç.æ?îõ'/Ep€?‡Ì:"•AÈ? ¦í	ñ*?‡Ì:"•AÈ?ﵨˤŒ?€MÙeV,ó?'•þŒfðð?€MÙeV,ó?å˜g^?Ñ/õàv?ÕÒÏ1ùCÆ?Ñ/õàv?íyۂêwû?¡C–Šsöm?´1#é3©?¡C–Šsöm?åMí…?½N"[?Õãeãè$ö?½N"[AGN4FGL J0609.0+2136c?ì6d}ØóÍ?ì'ÔžReþÀ9·¡I'CŠÀ;F"ôï*Æ@itû)¬w@
€™îS/?ȑ)]œhV?ØLv›gÏó@ê^ã»&?ëKÿ‡V˜¿ÓmˆÄŠ3¿â²âÀÔñß¿àJþ¥·à¿èÙÇÚñS¿ïþAÿ©ÃÞ¿ïó÷H¡YUNASNone3FGL J0609.3+2131?á?Cs'=?͇='
?݁yúۇ?͇='
?ÍÂË÷º·!?Æâ¶a. Ø?èMR8?Æâ¶a. Ø?çUU'Weu?¯…:_Hü"?ÑUU±Q5?¯…:_Hü"?Ð
z†­>?©cCülF?çú¼±)a?©cCülF?Éo9_J?Éàˆ‹ªB´?é¤1½è-{?Éàˆ‹ªB´?—´f'"í†?¥§x>%
Ä?ïB\˪ZS?¥§x>%
Ä?Æü¢û ?²ºâšL?êy@ÿWA8?²ºâšL?"'Y
°x?qÎÁ) ?ï¯aÊuYž?qÎÁ) $MIXED4FGL J0609.0+2006¿ÎoºS‰¦?Åd†gbºµÀ9i'¹'m-À:õè½ÄM@¯r2!I@z¼i¨:?Ô;âjØ?ã]0'oí@³?…Q
9@¯upðX¿Õ1Ä{¼¿Úâ;Þ}y¿éC¿rq6¤¿ë*†ñ÷(Á¿ïÿåþÌú¿ïŒbUNASNone?ã#};H?Ò¡]m¿?Øá鹉q?Ò¡]m¿?Ïôè·[mÜ?È7`Çô~u?èÅÒ)$‰?È7`Çô~u?æ{GNs*š?±ÃZÿ2?Ó	qcªÌ?±ÃZÿ2?Õ÷!½?±0×&Ě6?åx"o!19?±0×&Ě6?ÕwiÔ#¦?ÒkY/F>©?åDKýî-?ÒkY/F>©?—ÉuªQ!Ü?¥ç¼*u?ïA´R­vñ?¥ç¼*u?Ôøí½]?·Z\uíZ?åý‰!|R?·Z\uíZ?™^Äæ?nmÖO1?ïÁòÍ"Ä6?nmÖO1MIXED4FGL J0610.8-4911?è£ÓÍO²#À:–YòºÀ;˜=Çá¬À<Ñqk}&œ@!A'±tט?þÐæòèÀH?ÌåÚ9òÀ?q£x}…µä?«ÊD /9B@=^Wú?ï饠ÿˆ¿êŽß+t"¿äHZ!^Ÿs¿Ì‡ì]‹ÌQ¿êk[˜­
¿»€@­S8UNASNone?ïþ³
LÞo?&»±6Ìà?$Ï/c8¦Ð?&»±6Ìà?ïöÿ3Yý*?U
7H³!|?R˜È¬Œ?U
7H³!|?ïíãu…¾?d¦c\ç?bŠiÃŕ?d¦c\ç?ïýŠpö|
?ŽãfUÌþ?3¬y±vùê?ŽãfUÌþ?ïÿN´eo=?Ö6I‹bŸ?)n¨ç¼Ð?Ö6I‹bŸ?ïݒÙG?Á?z ¿ŠéV\?q6"a/"–?z ¿ŠéV\?ï˜Õ?oÔmx|2?aþEM抈?oÔmx|2?ïø-Ÿå&û?A%"éÈ?OI€ÙW•U?A%"éÈAGN4FGL J0611.4-4722¿ëþÔü¤´À:ÇÚÄçÀ;‹ûZu—À<¿a¥6†@ý?Ãdn?@$	å\Ë?Ó«ãH9Tµ?Äï"77y¿?îü®a|ǧ@'Góߋ@?îâ<À县ãØöT…"¿Üß|Ò¹uØ¿èDÔ «±Ÿ¿Ð6ɀ<%u¿ïÿHµ{wpUNASNone?ïüw.H'?5@€vÛLù?<G$¯rV?5@€vÛLù?ïö8ê4ð*?UlÛðî,?SŽ+ðÕZÝ?UlÛðî,?ïç%i­(ÿ?gÌÅY}­$?hږXVa@?gÌÅY}­$?ïüÐNü+N?#:ðÉGÛ?9}ˆHmœ¸?#:ðÉGÛ?ïü ­¨!û?=8f!`Ý?>ú'¨ò¦ž?=8f!`Ý?ïÙþbc?{Nýü1Ê?sÎì¦Ã?{Nýü1Ê?ïÅH_ù"?€.Ôº9Ð?}[Ð_¥>U?€.Ôº9Ð?ïï6Ñù1…?TÛ©þ¦m?`É-ärc}?TÛ©þ¦mAGN4FGL J0611.5-2918¿ìé¤lízSÀ4ñŸŒ¨À;:Z—%KÀ<¸'MKã-@O'M ð@¼ù jn3?Æ
)#ºÅ8¿"zÞåËmÉ?ÐQJ8ˆ@!SYÄAŽ¿ïÿ_Dä?ïò$	ʄ¿èL?^9Ç!¿áŸ©³`ë¿âø›AåR«¿××Àâ¯bUNASNone?ïÿ<ê¨;.?´!ÁS"T?b¦T@?´!ÁS"T?ïö½«¿?TS3¹¬è¹?R"¨i=ÍÀ?TS3¹¬è¹?ïó®˜%ȉ?eKŒ@£²Å?X¢Ï€4Þy?eKŒ@£²Å?ïþrœÞ%B?<»óí€?(Ö1bÁÞ?<»óí€?ïÿ1]'y·?õ²¬ÿù?ÔEÄhÔ?õ²¬ÿù?ïÚÜqj?{́‡¶
?r'ÇŒ÷ÂÀ?{́‡¶
?ïíÓ18/?rf<,#?b,Ί%)#?rf<,#?ïøåô³h?AüÛ+Kâ?Lh,KyÜS?AüÛ+KâAGN4FGL J0612.6+1520c?ïÊX5ÌÁ¿õûš—À9Òc+Hƒ'À;$ý
':@jüz9'@'BÛFã?Úð¬¥åØ7?݈Vü1Q@ˆ.›
³@ŠJÇ#–?ïiGâlÇ)?Ô¿tŠ˜¿êrÇ2Y ¿í¦grÕàr¿ïüsž]M¹¿Fz•ÈSÁHUNASNone?ï7SNÇj?¨r¾êZ(?™–@þà·?¨r¾êZ(?ä Á¦†P?ÍW
Ór?Ö¾|³Àóa?ÍW
Ór?립"÷X?¦þ¦y&¥?Áe	íÈ"¢?¦þ¦y&¥?ãÓâsZÉ-?°ð¡ˆ.?ØX;Jm¦?°ð¡ˆ.?è;¼]ƒ?̝ï'Xß?ÍÃωõ?̝ï'Xß?Àqïö6lg?ɦun°Ñˆ?ëã"rdæ?ɦun°Ñˆ?ßSGÓB!?·ÔÄ
Åü…?àVq\^ð?·ÔÄ
Åü…?¦žÁb‹e?'¦á_?î–"¥?'¦á_ MIXED4FGL J0613.1+1749c¿ÚûU,=†Ú¿µ¿¿¯>-À9T*:†åÀ;dØǬÒ@ˆuÒ4j@
0'|G?Ã1U¡Îò?´Fˆ"ùª?ñÓÿü¥­@˜,J¶²"?îޏ¢ŸÒ™¿äKb¿gßb¿é¶nfÔ¿éÔ¨c`øh¿ÛÅÓ~—µ"¿è{éOºRwUNASNone?ïíµ3¾ñ?bô5/Ûd"?bJÌP~ß5?bô5/Ûd"?ïÍÓ]?uœ5<3?yr–Öi7?uœ5<3?ïÂêJâ?"jÝÇW?ž þÕÃ?"jÝÇW?ï½Ýh¦\¡?bÅðHק?€ˆ¥Í!åè?bÅðHק?ïo|"æ8?"76¨&²ï?'|«Ëk?"76¨&²ï?î9ׄ-C'?±¾B2üí×?¬b‡¸àJ?±¾B2üí×?ìôE7Ó½?ªt«Á—íû?¸]Ö@<ð?ªt«Á—íû?í"ž:Æ®?£ú`86ï?·[qü'?£ú`86ï$AGN4FGL J0615.9+1416?Â^4Ûпòê1ç٘À:!<ªÀ;€Uu}ZŸ@©®Œð¾Ä@sÆßî?ÒMyšöë?à/‹^¿@
9™Üµx@`¶™Y­Æ¿áOuž'§¸¿ã5­–¦ ¿âöT…"RX¿íχ\€3—¿ïþÚH¶R?ïùv
£V²UNASNone?ëbc@'sž?Ēë+Ôçp?Âvrÿb1Š?Ēë+Ôçp?êMɉÌG?ÅõAq?ÆÈÙØÎã¨?ÅõAq?êþ²âã1
?§N;ÎÚ[?Ä4ts;Ù?§N;ÎÚ[?ìÊbÆ[o?¡ÿØÂî4x?¹¬ïaÍ$‹?¡ÿØÂî4x?á!{Äá4Ó?̜õÞWÓj?ݽv=–[?̜õÞWÓj?Àw§%BÈ?ÆÝ<Ø3Äd?ëâ6¼ïN?ÆÝ<Ø3Äd?ÓP`ºÙÚ?¸Ln‰Å?æWÏ¢ó"?¸Ln‰Å?Í~«<ëT?º'mY¹s˜?è¾ U0Å+?º'mY¹s˜MIXED4FGL J0616.5+2235?ì"JJZ@=õ~œ¾À7ÈE`\a*À9ÞÅFƍî@"ϝ"úh@R¢™ó[­?¸–¾»<,?¬ø@¡Žc8@ÂJ»5'@V¸­¿ïâ'x?܃ÒÝÝì/?ï^ˆ¶óF´¿Ú%р´¿â#πÜ3¿â"@^"àÍUNASNone?ë&Ì®!™‹?ȏR[x)?ÃdÍGy™Ó?ȏR[x)?îõ8$s¨?²b˜¦¥R? ¬~RH~?²b˜¦¥R?ä,'pncF?¶¨hKÓD	?צû#9t?¶¨hKÓD	?ìÍwâß?®5´—̺Ù?¹"Gp{ý?®5´—̺Ù?ì*靽ëˆ?¿ã§Ú¤ü¤?¾¨³£¼?¿ã§Ú¤ü¤?íXXHbç£?À°½]Õ.?µ==½V¶f?À°½]Õ.?è18w'?·Û³Ã!u?Ï;Â#aÀ?·Û³Ã!u?æ¨óåђ?ÄþÔ*$R?ÓÄ®4\Ý?ÄþÔ*$RAGN4FGL J0617.6-4028¿îø`ÌQÀ7Kğס<À:Y:Ütà}À<Aß®Pá@"ÁlFz8@²c/
°?Àâ2d¬'¿~9¡æܐ?´Œ•z%5@¿ê»Ë?èQ­DqI¿ã–ñH­¿éŸK¿ñò÷¿í-­LÔÄé¿ášß÷-É¿ïýVlô!UNASNone?ïÿ#
,e?Îrø(Ü?{—ß¡Qj?Îrø(Ü?ï÷aÒ>7?U(o'-«?Q<[pT)
?U(o'-«?ïàÁÇh½a?rt…8
¸z?o>8ºþŽ|?rt…8
¸z?ïÿÉzno>ë!çW±aç>ûBÉ¡/§Ž>ë!çW±aç?ïÿLXjœ£?º@†F?tñÇH1ñ?º@†F?ïއ^Ðè2?zëyš?p¼P¯™*÷?zëyš?ïÙyÈ?y°Ó|Q?s}Ã'&K?y°Ó|Q?ïÿMfÿØ,?˜'2y?SÊ%?˜'2yAGN4FGL J0618.7+1211¿ì¤‹t¬"¿ùvœ>ˆÀ9Žé#D¨¦À;G5>¦-ý@ʈzdØ@5½ÿªo«?ο<"÷?Øwîý`h@ëð«Ï?ýÏôÄã¿ÒÁÞݢĿâT‡@сg¿ê±  œX¿ïþ†¸ìE8¿î{qZ¶.ü?Þ>;Ú¡¡¦UNASNone?ïÈ°ÖY?3Î?'Ûø?{§ñßøkì?3Î?'Ûø?ìXôZQÒ}?Àn6cG?½8]-ql?Àn6cG?íŠ;‹O¬?ž|—€9Ì*?³®#¦Ñ¥?ž|—€9Ì*?íq"[Õ¿?˜jڍg²?´vì³^‹?˜jڍg²?ï@NÂ/åÌ?œ­'üìq¥?—ö'±l@'?œ­'üìq¥?ËGu¬Ìɔ?ÎX—¤25?é.""Ì͛?ÎX—¤25?ä:ߌ9"?µ³Ù Ø˜¬?׊@çŒý»?µ³Ù Ø˜¬?Ԧح'Ú?¼!ÅfjÜÜ?åú,"©7?¼!ÅfjÜÜMIXED4FGL J0618.9+2240c?ég"*GYä@díoڃoÀ8£$G%ŽÀ:V>hñ["@ä-;¢m@0;>šo'?υŠX‰?×E$>MÄ@h›€úfc@ØçÓ
ƒ¡¿ìŠÝ"3¿Ù_`"T"«¿Ò'¾+I¿æO_žÌ'¿ëá'fw-^¿êœöElUNASNone?˦asbxE?Ê@ˆ»ûÄ1?ég£'aï?Ê@ˆ»ûÄ1?Ð¥|£ä?É^Îø 7®?ç­Aòò.?É^Îø 7®?Ôÿқ÷J'?³D4'QË?倲Z¿?³D4'QË?ÓÈêîuê?³"±Ìm?æö
ˆÅ?³"±Ìm?©°zë/m¿?­ó‰PÖo(?îdøQ#ÍÔ?­ó‰PÖo(?œUa­ÛJ2?¯tå5GŒ;?ïTòu¨Ï?¯tå5GŒ;?±=Ž?+5¤?ŸKž†_Íg?íØN7ñ]ü?ŸKž†_Íg?º6_Ÿ
9?v"îŠiRb?ï¹&ž`?v"îŠiRb4PSR4FGL J0620.1+2246?èÁ÷îRrW@
º"¹À9W|i+À:ðÁëÈ:—@!`>Æ4W@F$<jÿ?ÄK©â,£?°Ø*ùÓÁ?óR¥ôñ¯?öí՚¦µ¿ïðÏ«¤^?ïÿ}ÄPýI¿è¦,Od¿àcuÏ¿ì×LbY;†¿±²à<–3^UNASNone?ïY4gC?ªèë‹T?"ÝYs¯?ªèë‹T?ìï^>éd?¾"Ú˜?¸‡-
,Íä?¾"Ú˜?ìYØ8À,?§ÜâMiJ?½1>;yþŸ?§ÜâMiJ?ëŸÌ=}0z?ª78ûo´?Á€Ï
>?ª78ûo´?í¯nI"¢†?²\¹'ÄË4?²"¶Ñ?²\¹'ÄË4?ãUܑ¢?Õ'ͧ>ü?ØßTFÜ»á?Õ'ͧ>ü?ë)­àfô?¬Ž,/â/…?ÃYHºd.?¬Ž,/â/…?֝$‰ÞKá?òoQO1?ä±m»Ú?òoQO1MIXED4FGL J0620.4+1445?¦ðÊ¥L¢'?l`ÃËW"À9ªu߀-¸À;LM++ýµ@¸¹Å^@F&}BJþ?Åʤ¾æ°#?¼X̔m¶?÷pd·9½'@´Áº ,?ïÌÝÉtR¸¿ã¡fµN+¿è=Ëݹ"¿ç_™Ã‹«¿ãË£l2›¿ïÿ!}ÿ	`UNASNone?ï÷]¼k"/?MèˆÌȄ?QD†òÁá´?MèˆÌȄ?ïÚKù±9ý?{Œj £?rÚFO}h?{Œj £?ï϶›ªba?y¢Q̗ò÷?x$²*ãv?y¢Q̗ò÷?ïÏNJ…'?Wº¬PÜ?xXÚØðCå?Wº¬PÜ?ïõòÚõÑË?O떴B?TI±gª(?O떴B?î˙½<L?¬²Ö®,`¢?£Fd.Ñð:?¬²Ö®,`¢?îê±,æÆ?™¡`Ìzk?¡_"èæž?™¡`Ìzk?îh¹É +*?'±ÏwJZ?©tcqlé]?'±ÏwJZAGN4FGL J0620.7-5034?×®NŠ°%UÀ9Q—ÃքÀ;•æR¯Ð=À<ä1Uãad@!s?Lœì?³IWaæ¤å?âøVCæ?ï÷q@ŠØ?øAÔ¶¦@J=g>¨‡¿ïùæÁ²À?ï}4ßݵ¿ëG¾Ûr'¿ÏkZXæ÷¿ÓkÁ¹É:¿é)g7F¾*UNASNone?ïýŒ>«ü?nbóFÂ?3žÈýá ?nbóFÂ?ïö­¬~¬6?U¼Žî:?R¤§#£ÓÄ?U¼Žî:?ï¯mýæ?|‰šuÈH?"$›ÅŠºŒ?|‰šuÈH?ïþ¿kÃÑ?<V¤	mL?$	Bí¡¦c?<V¤	mL?ïû˜–Kí?Fõ7ŠLW?A½¾?Fõ7ŠLW?ïÛð‹©þ?{°iyçx?r~Á
8ø?{°iyçx?=gÙG?ˆçŸLf)
?ˆYð"Û¢[?ˆçŸLf)
?ïÿN¤Ó´s?!šó€kÖ?+mä§e9?!šó€kÖAGN4FGL J0620.9+2201?¾¬úý°@/ !·"À:íFƒrèÀ<º&‰@$d/€ KÐ?ø÷3"«C?Ǽõ©ºÎó¿ŸÔ€Âªk?ÕQÓ1jÜ@Vô²ný¿ïÏJöžWn¿ÐÐM_Ú08?ïývþ«¿èÁ€}éºÄ¿Ì"O
TAÌ?±£až²UNASNone?ïÿmXûÔ?ÉlÙ£À?Të™eNé?ÉlÙ£À?ïê…}éöå?sl4'I?ezõÚÍ?sl4'I?ïë°µ"÷É?j•táž?dOJ‡äîˆ?j•táž?ïûïämÂ?7T¶zJÕÙ?@@mÜ©™?7T¶zJÕÙ?ïÿVQO9?«øÕÙ!ý??­É,'0?«øÕÙ!ý?ïIÛýRŒÑ?¥0Ð{"ºø?–Ä€Sö—ä?¥0Ð{"ºø?ïá"!ñu?wPÛÁNJ?nÝÞ$ˆ|?wPÛÁNJ?ïöŸmdÌ?P§D0À??RÀßCr÷"?P§D0À?AGN4FGL J0622.5+3120?íV°ó
²@ K£ÂˆÀ:*3°1À;»©É'†@¦",0‹@žÜ~ñw§?Ñ`šŸ~
?妟Ԝ$@âZÛGº@ÉîvÚ?ïÛ·`Ô×?åå[¤k"³¿ã¸¥bûwÛ¿í͂iÒ+±¿î
^þ"¿ïý'AŽ?ÉUNASNone?íßÌØ›£?·«Ñrà?±™>G;è?·«Ñrà?êz=Hr"?õ6ºô'?Æ	úÞ5³?õ6ºô'?êíqٝPï?¨A#$·?ÄJ8™Š¼B?¨A#$·?ä¸|Ìaös?³Û¸<Í?֏g<?³Û¸<Í?ä巖sŽ1?ÆÒØ%V·Ù?Ö4Óãž?ÆÒØ%V·Ù?Ùj1³<"?Ò'±ó‹0(?ãxJç&a¶?Ò'±ó‹0(?á{ :Ù«ê?¹0T›2¬î?Ý¿ŠL¨-?¹0T›2¬î?ɛY±»é?±¡Ÿ`»©$?é™)"'»?±¡Ÿ`»©$MIXED4FGL J0624.7-4903?îؑԩ:!À8U»YÝÁèÀ:Õ}<kÁÀ<…´Eâb@òàY@@×Or.Å?Ð^Wú?ÔXsÉü7ô?þø_<¦y|?ÿÃVçmb¿âC"×ü¿Ü·ØIё¿ç›ÁýeñÌ¿çè"M×ú'¿ð?ïþª*
•…UNASNone?ïÞê.°í?l'¸Ú @?pŠö\HñX?l'¸Ú @?ïٔÍƶ¢?û'–+â?s5™*cì?û'–+â?îrAMI¬>?™ÎÊ`³_?¨Ûë,A#!?™ÎÊ`³_?ïÖe?aÀÿzy7?tÍ90Y®W?aÀÿzy7?ïÈé`9ô?|¹PKxuœ?{‹pHSâ?|¹PKxuœ?î¯àx®Æ?²>ޑ_'G?¥øu?²>ޑ_'G?í^g¡FX¡?¢"6ڐn?µÂôñS÷?¢"6ڐn?s_¯?¡ØÉúóAO?¯ö$uZi?¡ØÉúóAOAGN4FGL J0625.5+7029?íy[bɛ6@7Y±ú¹o"À;ªçä€G¹À=µj°x@!jÄ@?ú±´"#˜?Ô;CMÄ?ÊI¢¶MÚS?õ‹Íþûô@‹=8ÌÛ¿ïÿâÙ~‹÷?ïÿúŒ—Ó¿èÞ*o¿yî葵†¿à]½Ž–[¿åª[Þ£
UNASNone?ïûzö§wå?D¼é&gÚ?B%OoYª?D¼é&gÚ?ïð!ÍI
T?a4¢BæQª?_¼e]g8B?a4¢BæQª?ツE"@?€¯c•†¦?€_y>-­Ð?€¯c•†¦?ïïhkáË?GÒM÷u?`—"d-'?GÒM÷u?ïüu¤ûU)?7±&óó£ï?<R×ã^84?7±&óó£ï?VšŽê?‡^J'j?€ÒYiSÜÆ?‡^J'j?ï¥RH]x?‰{cCÖN?†«mï3›?‰{cCÖN?ï³=s(?vÉ%µàŽÙ?ƒ90¡Ö"?vÉ%µàŽÙAGN4FGL J0631.0+5626¿©­A
D#1@3¥õß덂À;-DÏ<é•À<ÁŽêéîF@çÁÑ;?ÿúü‹z?ÑaæåQÓÝ?ӗ­µ°@Á[šZ‰¹?þ²Í‡²¼U¿ïàîzÔ]?ïF"y&²?̃K쓿Þ>˜â9›'¿é6Í0ŸÛ¿ïÿúŒ—ÓUNASNone?ïÜL/8÷?k›+"A@6?qÙèeð¸?k›+"A@6?ï4Xù&®&?Ÿ¦r‹†Þ
?™tàâ	s<?Ÿ¦r‹†Þ
?ïfCò%ÕZ?†Þp•À?"7¶ê¿?†Þp•À?î6óõ/Âe?‡ÙÉVˆ=?¬À­Ù©?‡ÙÉVˆ=?ïŒ:ä‹
?†IîÁ?ŒñFÒíæ1?†IîÁ?ìÀƒ§®žþ?ÀÓwÙ!ç?¹ûâ‹?ÀÓwÙ!ç?í;º6®N?£¨×
¹?¶".IC´Ã?£¨×
¹?èŒMAë÷y?±5Ú*áß?ÍÎÊøP"?±5Ú*áßAGN4FGL J0632.7+1215?Ú1{U¿X?÷¦Kç_À:
á'ï¤À;†}=B€®@"'Ñÿ;µ@&eÅV·?Ëc¬¢µÍ?Ô
"þLf@	"•á~4¹@ƒwçî¿»Tÿá¢ô¿Ïxbmοæn'¾-øŒ¿ågµñ¾ô¿ïÿþˆ0»Š¿Ì<Vžó UNASNone?íhE
Ñ$?±8iÀóV£?³ô½ÖGœb?±8iÀóV£?ëÁæê&Ç7?¿§n%nñÈ?ÀødWdã&?¿§n%nñÈ?íG1'aUŸ? §¶=|ó?µÆstl? §¶=|ó?í ,_¦Ñ?Ž<H^'N?²þ7kG?Ž<H^'N?ç76L,¯?Á§È¹ö9?ё"gó¦£?Á§È¹ö9?ɦ»O:¿ˆ?Ìõ²8Ö?é–Q,1P?Ìõ²8Ö?ß«·àß7?¹ã)3ïµt?à*$÷e?¹ã)3ïµt?Ø~ÝN,çG?³»!êæ‡?ãÀ'XéŒ\?³»!êæ‡MIXED4FGL J0633.9+5840?ì;™)mj@4¾™A…ŽÀ;dûHábÀ<Õ±·Ÿ@ 	ËÚŸŒ@ÎÓš3ó?ŧ`Ÿý·?À­ëÇJ?ÂQœÀ? ª@ñ,}ŒrÀ?ïÈW¢~D©¿àW@Žeˆñ¿ä t´Ý¾¿á I·6ì¿ß‰ˆª^ü¿Ô´4iq3UNASNone?ïüþý1Õ¡?)´×É{Î?8úWÉ?)´×É{Î?ïò¯?ѯ¾?[§®3ÊQÜ?Z¡€›ÙS[?[§®3ÊQÜ?ïóŠ»=r?Jíœ|Ɠ&?Xê‰kQ?Jíœ|Ɠ&?ïôIU´g{?7äµà‡85?WmTÖiÙ6?7äµà‡85?ïûé-øÙ?8{Ýi"¾|?C¸[ó¢´e?8{Ýi"¾|?ïÅÃbY«1?‡Dk"Ï?}NÌû™?‡Dk"Ï?ïïÉâ•>Ÿ?jèØì̹°?`6Sd	w?jèØì̹°?ïÈ·¤úÿC?gš•PŠ`?{¤-†Ÿæ–?gš•PŠ`AGN4FGL J0634.6-3046c?é¨"EÐÝÀ0Ï8£µ|NÀ:8WšÀ<DOúêŠ@¶Ñ"@ÈòZ%"?ÃyR¼»\¸?׏=Ë·?õ#ºð+w@qµ_ðý¿¾²»(µ€Ö¿å«;þ/¿ì¥• æ"õ¿àê¢Àß®§¿ê˾ßK¿ïÿøÞ£ŽæUNASNone?ïݚ,'ƒv?uù…Bl²–?q2éË,?uù…Bl²–?ïéª/¶Hs?s&^>cq?fUÐj³Ìz?s&^>cq?ïœÔ¢J?âûý'?ˆÊ׌ë̜?âûý'?ï܋^ms¡?X¡
t9?qºPÅ&§•?X¡
t9?ïRݿۚ?˜7_ܗB?•¤HÔïÒ?˜7_ܗB?ï§7òhE?Ž[ÙÑ\?†92
´Â—?Ž[ÙÑ\?îR_'{†ù?žì•=õ?ªÚÕ³Ûw?žì•=õ?î»XÈ1÷8?'/÷J—w?¤Js€P(?'/÷J—w AGN4FGL J0640.9-5204¿ì]9ů³HÀ6Ÿ(ǟfbÀ;Ì
V)ØAÀ<ê?ÉC«P@ Éí
4?þáÁçâÓ?ÛÚ-þ•ò›?²ÞÐZuíB?ÚÂÑ84$@	Î{"¶
¿ïü3ŒõFi?ïþ^‡tÔ¿çQ°''¾¿â?bžÍ¶¿V"ì"q¿ðUNASNone?ïÿ`åh?%ÞµãÑÜ?¨FÕã¡?%ÞµãÑÜ?ïöÚ»´é?V=auÀë?RJˆ4ýY?V=auÀë?ïêû1(?oDU'ÏB??eå}ДÈD?oDU'ÏB??ïÿ¸šÄDœ>õM@ùt¦"?Ù@_Vì>õM@ùt¦"?ïÿÀߦÁ?ÔkôWÔÇ>ÿ#Eݒg?ÔkôWÔÇ?ïÜn+'ç	?{ ÍȺ?qÈê5,£r?{ ÍȺ?ïä¿­Öà?u§rÝK?k@üz˜?u§rÝK?ïþ½
̍?#Ä´Wߪã?$/,Šlëê?#Ä´WߪãAGN4FGL J0642.4+1048?Õÿ…)R½E@{XÑRm‹À9ïL}‡\À;'Z5Ö{¢@‡åÇÅ{ö@F¿Ä§?ɐ]b²?ÖIí{ì
@>)#øÁ@TbCÁö°?ïä©B."Ó¿ßÄøÂôܶ¿é¼O§@¿çòáԛÎ'¿ïÿùSt?ïø#ÝÕ³¦UNASNone?ïÂcÛ=J?+hq\Ð?~Î{ŠÒ6Ý?+hq\Ð?ï£dÿ3&s?"­ÿýÝ®?‡&À"WV?"­ÿýÝ®?î׏Äμ?'r&ç_#?¢‡ÃB°5?'r&ç_#?齃Òä?lß<Uæ¥]?…;Ç×cŒ?lß<Uæ¥]?ï
óŠ7?¥wZ'ª?þ¡"àˆq?¥wZ'ª?êGç0^?É`h)–?ÇâàcÇ>‡?É`h)–?ë›Â‡_Ám?©•5ºT­µ?Áõâ€úM?©•5ºT­µ?ëΙ5²?©ù\¹®Û?Àś+ñ9?©ù\¹®ÛAGN4FGL J0642.9-6501?Ì"1°Hª
À9L[9âyÝÀ:‹¾‰=+À<gñx7@qGÛ
þ@¬ÂPr[?È«k=»¢X?²6ÊA'+i?ãEºßd@Ù¢.¾"`¿àûs¾¾—*¿âº›aÅ¿çvx݌b¤¿ã'eMa²¢¿ïÿ¾&@Üi?Á#%^‰MFUNASNone?ïù¨?@E?AËܵÁ¤?I_0
-±?AËܵÁ¤?ïôÀh²¾P?Yl*1ëè?V.¢Âo¡?Yl*1ëè?ïàö'?eÐ¥Âg‡?oîéØQ#?eÐ¥Âg‡?ïö2ÒVà??^ö¬À©?Sš[ªX€5??^ö¬À©?ïùτ§¢?D¸ŒæIÞ?HÁïi—P1?D¸ŒæIÞ?ïÔM&ÏL¯?~Ã/þ=
?uÙl…Ø®?~Ã/þ=
?ïØ8p‰Õ×?zf«C±ÎÎ?sãÇԂ0A?zf«C±ÎÎ?ï»úÁP?r&0#/ñ:?zþGÉæ?r&0#/ñ:AGN4FGL J0648.6-3623?ã%'ƒLÀ07jøœ^pÀ:ÐrûÀ<A5" ¼8@û˜‰y:ÿ@ù—"ÆÔe?ÕGwB¬¢á?Ö~<ЕÚ@Þò"z–@%xÄ¥?ïgF€l÷пã"E	Œ³¿å/Gì'Ü¿ê;ÔÂd"¿á—½¡`¸R¿ïÿþó…õUNASNone?ïì»ô¯Ï?]Dz©?cD«J?]Dz©?ïàê÷É4?ráµAûÙ?o´/K5?ráµAûÙ?ï_rÆã?Š ºÃ\w?"¬B9£?Š ºÃ\w?ïË׺²€?^Áig C?z"Þé@?^Áig C?ïâÈBŠ¥F?nˤŠŒ¬
?m7½P>ò?nˤŠŒ¬
?ïk	Œ#lõ?›g¹o_Å?'žÎ€¹ËT?›g¹o_Å?íŽ݆¿ˆ?¤ÕîìSÈ!?³ù¤B??¤ÕîìSÈ!?éu?"«¤_Ј	?§7"-¨?"«¤_Ј	AGN4FGL J0650.2-5144¿ê±4ÝF0€À5'	"ãÿïÀ:â$GÝå#À<ž¡ü>ª`@!N
©§-×?øñ¤óið?ҋ‹#ŠÑ?Í5Táä·?û±¾‰=+@†+ëÁ.´?ïúöv'"¿íx¾W¿¿×ÉA|¢¿×Û;Û"zÿ¿Ý;ƒ"…F¿Øƪß<;UNASNone?ïûڐs™ï?1̇ÿa/é?@•¾wö¨J?1̇ÿa/é?ïó¤¿ñ?Zû8—4ˆH?YóÐd	~?Zû8—4ˆH?ïß°œ6ú5?jU¬Ãa¥ø?p'±ÜCÕÈ?jU¬Ãa¥ø?ïé;®6?Is(
ƒ Ê?fÄíLJŽ ?Is(
ƒ Ê?ïûÚXó=?9²b9w?@–\8{?9²b9w?ïÒ|*.8?~´Ñýdúi?vÁêÉ÷€6?~´Ñýdúi?ïÞ砍ª?ty¬'œ²?pýƒL?ty¬'œ²?ï´ìYÁ"±?p'ó†ûªV?'Äééæ?p'ó†ûªVAGN4FGL J0651.9-4330¿ÐZü$ÿÀ24GñQçÀ:Ò¢ªºSNÀ<K Ÿ²¸@¶å‹Š7@jUp
?ÖĶv$J?â³7É
û?ýDr‹7×@
M"¿ä|m¾I|¿Ñ!åBq£¿è%–ýÝæÑ¿ïö¶?¯?îœÏä¯A¢¿Ëg!!bÑ1UNASNone?ïüR»'¢ ?DrÁUÁ?=j(t #S?DrÁUÁ?ïôŒxw?XÝx2Ñ"?VæŎ˜sO?XÝx2Ñ"?ï=>ª4Ç]?Š3ý—÷¬??˜X*·¯Fd?Š3ý—÷¬??ïÿ#fŒ{ú?îWR7ûË?"'ÓAO½?îWR7ûË?ï÷Ï#-"?`*`ÕƄ(?Pa¹ƒnßÝ?`*`ÕƄ(?ïÁ€¡È_?Š
梪È?s¿¼Ú@?Š
梪È?í¢õšO?£=o÷.¬-?²ï`Qw·Š?£=o÷.¬-?ïç'SÖì¶?mxLÉ°ƒX?hج5qá£?mxLÉ°ƒXAGN4FGL J0652.8-1855¿è>ö«¡±À jÑÐAÌSÀ:¤V¦ÖÀ;¬ƒ•KV@@™vÈß,v@±«Vç?Î3[!8ßÅ?ÇFM^;J?÷b¢Œ‡b_@¯ãËh?ïÛ †ó¥¿äÒ¬9¯N¿äÕK@ÆÔ¿êäÞבL¿ïó¾ýq?•¦í}XUNASNone?ïßø×i°?~O¬±ërD?p"Y»÷?~O¬±ërD?ïÑÿ
G*?}ÐlÒ?wuen¯	?}ÐlÒ?ïIğś?ŠVñûƺƒ?–Óv"Ž?ŠVñûƺƒ?ï‹á6ޅÔ?nÔ®c©?²YŒ–Ú?nÔ®c©?ït­6¸–?ŽÜWO	b?'jY'HR?ŽÜWO	b?ï+`0¨?¥g]³ï™?žúõ±¸î?¥g]³ï™?éÓ­
Œ'
?´@Ê0bm?ȱKÉÏcÍ?´@Ê0bm?ì$´¥í¤?¢xï,­Ží?¾ÚZЗBã?¢xï,­ŽíAGN4FGL J0654.0-4658?äp,·²Î
À3
#Ä*fÜÀ;ja©ÊÀ<Y­}|,¡@yåŸ+ª@ù7ªÉm?Ãr(üÎr>¿±€ð«NLê?íçAÃîä@ƒÃvŒÏ1?íVþ–¶¿êŽ|/%‡¿×Jä•@n…¿ìg«ud0+?½ÍË`¢=h¿âŽ9žÝ%`UNASNone?ïý=¼èÂæ?0§ÝšÁ­B?6'_Ï?0§ÝšÁ­B?ïó'û³Á?\BÎFu‹m?XÜ	š]ä?\BÎFu‹m?ïÊ_nð?}IÂG¶î?zöPf»D?}IÂG¶î?ïüÛÈç?*
»9ç1!?9'ÙS›ÍÌ?*
»9ç1!?ïòð|C6O?Wy(ù/?ZJر?Wy(ù/?ïÎ[ðÁž›?€ñk
OSç?xÒ¨®C?€ñk
OSç?ï¦ë+)ù?ˆOÄyÇ5A?†E59(ÝÈ?ˆOÄyÇ5A?ïÙå·ÝÚð?nž'þOa?s
#ý$ÌE?nž'þOaAGN4FGL J0656.5+4218¿·¦äw6¸ç@2ÄÓ¿/UXÀ:û
ìQÍRÀ<~܏¸oH@ êÝïßÌ?ýÚy°Æ?ˑ<ÓÅåR?Ƙf?Ïú?üvÕIs™@€ž'&ޑ?痢–'R¿à'ƁY0ô¿³ðýmZ¿Ú7Ûu¼Æ¿æšaÙ¿Ï×æ'öÀUNASNone?ïüŠÉï*?1YÌ,zæ?;¯YÈ·O?1YÌ,zæ?ïå"×	‰
?j:LPìNÄ?jk(¸û/?j:LPìNÄ?ïëÿ?ï6ã?^L'À±Å?dÀ)†M@?^L'À±Å?ï¡þ{¼¿?eÉ/) ?‡€aAü<?eÉ/) ?ïøÝ~´Ä?D"O|xàÇ?L‹šÛ"Œÿ?D"O|xàÇ?ïš
²< ?'Bl7ëç‹?‰|"{&Ͼ?'Bl7ëç‹?ïÕÁÒë[?z§vkŠK?uhȦ'?z§vkŠK?îvp-JÍ?Éz¯_ä?¨˜ý-æã¼?Éz¯_äAGN4FGL J0657.4-4658?é‰}†'TÀ2'¶|(o‹À:ÈÈðŸ:À<›7W…"@Ý)ÆøÍ\?ýËj|uœd?Ì<>Y'?ß<Öàvø°@
¿Þd¤ÅG@Ia}žf]?éù¹à?Óë{#6æÇ¿Ø«€ÁF¿àå½^šÀ¿ïþ°_-âç¿è1ö½aÿUNASNone3FGL J0657.6-4701?î-ZÐiŠ?­fŸÎb·?­*Rþ™g^?­fŸÎb·?î* ‡Êd=?«-˜Æ^>g?­U÷ƒY¼4?«-˜Æ^>g?ëˆùXˆ?©ˆOå"(?ÁÜŸµßÃ?©ˆOå"(?ìñs 5À?–΍[®#?¿HtbþR?–΍[®#?æÐXVV?ąÅ}p?Ò_OÏSÃT?ąÅ}p?å¦Cù©ú?Íç5ƒÅqå?Ô³x¬
à?Íç5ƒÅqå?ÔÕ$EjÔp?ÁàŤÂö?å•mÝJ•È?ÁàŤÂö?átÏ;¬?´«9[節?ÝÍôaˆ¨?´«9[節MIXED4FGL J0658.7+2318¿à9Ò	Þ·A@'Ñ"D¿À:Ï-˜¿À<eÅööq@&=Kþ@غ@Ù$?¸5%¦­©¿'µÜïB?·/ù‰@ѾÎ]?îÝ)4­¿àø»Ó€E5¿çË¿m"¬¿äsšA	_¥¿ãbá@øÔ¿Ò&c«KžUNASNone3FGL J0658.8+2318?ïýÕУéK?"~¼|Ü|?1Q|‰ýü?"~¼|Ü|?ïð?g7á]?c°™70ö?_1	Œ—?c°™70ö?ïõ,‹r1?HTª?éü?U§øãœ>/?HTª?éü?ïú3I¥ÝÂ?*6/–Ü?G2Ù-¶?*6/–Ü?ïü1Œ.?3€ï÷–±?;‡Îá'??3€ï÷–±?ï§FÜ;q?ýòcÔ?†.Hàó?ýòcÔ?ïí«r<»ü?lÚ(GúB	?bT†Êä²?lÚ(GúB	?ïãôÈ®ú?WôܙH?l7*Žb?WôܙHAGN4FGL J0700.2-5118¿éI×SRQÀ3‰æÿ}úÀ:ü`8NûçÀ< !¥l5³@—€Ã^äè@óû¶Å$?ÈW2ÁÉ8™?ºäù}º–?ð] ½é¨?õs˜Ôw¼?ïû¿ß(™ý¿àCòÖKҿҁ~ƒ=¸¿äÐeÁ•a¿ïÝUE¬²{?îíŽ]ü4™UNASNone?ïô"M?SødMX´?Wýݒ¢†?SødMX´?ïÂ=&H‹?‰Û5†¤¾I?~álîø+?‰Û5†¤¾I?ï*-ã4¡?'Ê•°˜ô	?šºC›%ÙÛ?'Ê•°˜ô	?ïeÿ¥ßo‰?|kâ•K­.?"@BZ@ß?|kâ•K­.?ïïC_®ÄØ?`NƒÓSm?`¼ dxøR?`NƒÓSm?ÏHÊl?«0:gÝÍ?¤SO@E?«0:gÝÍ?ï*æ9Ó?"éɤZ?œÚ¾dð"¨?"éɤZ?ì°cR5?©Ò¼âS?¿büånY?©Ò¼âSAGN4FGL J0700.4-4308¿ÞVœ€À0¤a¶Ô=À:ž;¼n°¸À<AäMòÒ@ý¦kd@8—Ü*7â?ÄÆFuÛ#}?™|cÓ¹ü?ÐԁLá@©zJP?×,B®{S¿åV«€'¿îÆ!·à¬¿¢	_$RÅ ¿ïÿÿ" 5•?ïó@oܲUNASNone?ïñ#™À¹w?Yˆg#ñèã?]¸Ì½Åâ:?Yˆg#ñèã?ïôš²&
?XèÛ{²B#?VʛH¶E?XèÛ{²B#?ï°=³Ðã™?~R¸çÄ7?ƒð'ü¨ÑÖ?~R¸çÄ7?ïûdº•µ?1©ž˜?BoÐ냼?1©ž˜?ïÙµ 'M£?s'€|"cf?s%oØUn(?s'€|"cf?ïÑT­¬·?€Á¸ë›#o?wU©kzøœ?€Á¸ë›#o?ïŸÒÓC€Ö?†Ä‡´ç¨?ˆK<Þ:…?†Ä‡´ç¨?ïÕn˜'?mn_WÌB?uqÈÐÙî¿?mn_WÌBAGN4FGL J0700.6+3558?鍛'Ž@1Cð#éêÀ:¾í¥Šh¤À<…˜f"³@þBƒ2O?ÿ'
;Qå¦?ËB%ŠÌ?Ø#ïÞʦ,@
9'N"¢Â?ýNÀ'"ß?ì'JSá)¿Ðè=µ¿ÜÞÝÛèɃ¿å¬•õ *­¿í`Ÿb0vÀ¿ïþ~á•›UNASNone3FGL J0700.6+3557?<'¼è?¤{àà¥Ó¬?¦‡ì6Jˆ?¤{àà¥Ó¬?ëãµäuWg?º³)^YbÙ?Àq(n*¢b?º³)^YbÙ?í•÷î0@?‹y2(Ä?³P@7?‹y2(Ä?ëȜݭ?–¿…Ÿ8Ua?À݌‰KÿÄ?–¿…Ÿ8Ua?ì·¼IÇÊ/?µ%´Àµ"?ºB±Á®Œ?µ%´Àµ"?×ûÄB‡?Ï¿á_‰†?äÞ¼}?Ï¿á_‰†?彧Ô?¹Ð1èk ?Ԅ±ãðÞX?¹Ð1èk ?ÞÂ;•=¥Ž?±ï{L¢Q?àžâ5a-9?±ï{L¢QMIXED4FGL J0700.8+1551?Ð<Ó­3 á@"^ËtÝønÀ:ÕZ±&~À<u˕•(@›Ãl{Ô7?û6KÄúp?ÓoI#Šs·?ܪù=n˜@Õe!ÂÈg?ýiÀÆY@8?ïøc‰<TD¿Õ×u1ÛD_¿£âï#
÷¿Ümz÷÷ž¿èƒÜ=®l¿ïÿËÝcßUNASNone?ïçaIWH"?fÈì<Yš¢?hž¶‡»ž›?fÈì<Yš¢?îô_ò?3X?¢O~|ä€h? ºÙy†?¢O~|ä€h?ïDؕ¾ÿÁ?0r=Ô?—díH æ?0r=Ô?í]ŸcÄ0Ø?ÕÊ$æd/?µ߸·Â?ÕÊ$æd/?ïd«Žð7?""˜—Yþ?"jÙÇ?""˜—Yþ?éÂó×J!?ÈúE+b?È÷è0¢×}?ÈúE+b?íd˜
xSú?¤¢SÂí??´Û?«Ïl³?¤¢SÂí??çÁ¦ _©?®@=ÐΗ±?Ðä|²¿@®?®@=ÐΗ±AGN4FGL J0701.3-0403¿ã셾½P?ÕÏæݚ$"À9dYbqå À;BöÜjς@aR½è@Rr†/YŠ?Æ-¡º$?Ͳt†åŒâ@%ÏÅ¥'?ûPü#ý`>?îèŒEô?Ð)ú¥M,¿ênar
ßW¿è"»ìª¸¦¿ïý ‡_r¿àÕ,ß?–UNASNone?ï/Õ"å:à?œ|¥C{?š[œykþ?œ|¥C{?è§ZU¶I?ÅZ^ï]¬?Íb–«±&Ý?ÅZ^ï]¬?펾c…?ŸÍuázü?³ŠDð#?ŸÍuázü?èöƒn×E™?¥	i¦°Û	?Ì%òD¢éœ?¥	i¦°Û	?áÞ$Dû)#?Í@¦EEü±?ÜC·v	­º?Í@¦EEü±?ÃÜ>FGô?Ê7"Ý(K?ëú0nn?Ê7"Ý(K?à…ÄXÆ%û?ºÐ	'µ§l?ÞôwNs´
?ºÐ	'µ§l?É%wÎ~±?©Ër÷ǶÞ?鶢>Œ`T?©Ër÷ǶÞMIXED4FGL J0701.5-2842?Ü¢;6@YÀ%GOøe×ËÀ:ûІ•°×À<CgUy¯@lþáòο@Y™~Á¦ÿ?É<Õ"oß¿›'Z¹gž?Òo_Éî@×~I1!`?ïݬþüõ?£`,¡¯ÎË¿ê§ýuDØ¿âTÁ"tŸ¿Ò‰À¾Kª£¿âª†7"ëUNASNone?ïýhwý›?-.U¦'œ?4¿úӏ?-.U¦'œ?ïóís>È?[@0IÜ[x?X%—?ä?[@0IÜ[x?ïäýžYz?rëâ(Œ
Å?kû\'%?rëâ(Œ
Å?ïüìWV©?!ú‰ìUŋ?8Cø"3?!ú‰ìUŋ?ïñ‡°t7Æ?aÚã™u?\ðŸ}Dâ{?aÚã™u?ïϵÔ|ˆV?n.<ñ{m?x%¬nAT?n.<ñ{m?ïÆÌÝ`:J?Â£rGá?|™'Ub;?Â£rGá?ï쓵»?Wã'á?clJ¼Ëҙ?Wã'áAGN4FGL J0704.3-4829?Ô orZÀ1ô$¢v·íÀ:º¶â¼yÀ<V "oeé@ ]¾!8_?ÿoÕ`EK?Ìvô©	Ï?¶vS€ÕS?ìki¥¶Ž@ëuró½|¿ïñ±ôr{?ï÷á]¨|¶¿çi2(q8R¿Ò±K¼ìÚß¿åžbP2¿ådi×4.ÜUNASNone3FGL J0704.3-4828?ïÿ'­!"X?ŽCSX)?TÄ4q'?ŽCSX)?ïõ6³ùʺ?XŽ´¼v?U'—¡6»è?XŽ´¼v?ïø;;¦…w?;Ø;WÿLO?Oºd
4?;Ø;WÿLO?ïù>°Ègì?3jæ]&Ø?K=ゟA?3jæ]&Ø?ïÿ¥Óp?ÀPÿé©?‹;‡ägâ?ÀPÿé©?ï×_V–~v?}­ÿø!Õ?tPTÁ\ù?}­ÿø!Õ?ïø¶®Ù?W}2¬ŒÒÂ?O¹%dôÄ?W}2¬ŒÒÂ?ïãýN†%?`r@3~·?l±jےü?`r@3~·AGN4FGL J0705.8-0004?á$÷ä±#@	\[cÓåÀ:"Ö¼À;¾7¹ª±@¥pŠí@¹÷<âß^?ÊàÓnu)?ÕYâµí7@ñžBuÆ?ü¹¼yÃep?²Áýäê%?ï\ÂMÂÖ¿âQ%!!¸·¿éè¢ì(²§¿ïì7Ì'ã?îi,êCÖUNASNone3FGL J0705.7-0006?ïNˆ±"âü?"árȵÁ?–.éҋ
‡?"árȵÁ?ëÕúã¶sD?Àu«…Y?À¨q&2ð?Àu«…Y?ì}€·9V?¢ºÐº²?¼ÓúF5L?¢ºÐº²?ëbaÛ"Œ?¤AÎÞ!?Âvx"uÏ?¤AÎÞ!?腺Ý3e?ÁêFi_®Ö?Íé‹Ó2m?ÁêFi_®Ö?Ф鏷SÐ?ÐÉĐyp•?筋8$V?ÐÉĐyp•?â+³Äàfª?¹,HU«Äo?Û¨˜v?2¬?¹,HU«Äo?Ò]ŸO]'´?·Ë+ž$©ê?æÑ0XQ>¦?·Ë+ž$©êMIXED4FGL J0708.6+1747¿äÎy…eý@'k͚R&>À:íÚü:x¢À<c;8»2@ ‹34à²]?þ{®—WŸú?Ð6[œ2ü?¶2ðÞ¤æ?ꖉ1+?ÿB¥Áðü¿îÉÔž›·?ïý¨6ëN˜¿å-ë?ÿtj¿àȖg"N¿×R[ø#h¿åû®Í…/UNASNone3FGL J0708.7+1747?ïþ¤»‹±Ï?9¤hL¤ã?%´Jg‡ÄŸ?9¤hL¤ã?ïãJMè&?w6À•‹´Ö?lµ²J³·?w6À•‹´Ö?ïð·3øð?_ Í¢ÛÌ?^'—æ'Ðå?_ Í¢ÛÌ?ïçTŒc?P0|¸?h«sZóp?P0|¸?ïþmË#n3?!ãȲ­º?)#QWåC?!ãȲ­º?ïJãå(tz?£VGÉ
Æ?–£ƒ^aÊ?£VGÉ
Æ?ïñ²ÈûÃ?f"¸Ä…•?]úšGŒÚ
?f"¸Ä…•?ïuHiPP¥?ÏD]ì\?'VòÔ>W?ÏD]ì\AGN4FGL J0709.1-1034c¿Ñjfõœ=¨¿íKÒ»úÀ9!ÌzdJÀ;1œ_F·t@üx±—'-@ÁåGíÕ? y‡«ZŒ?ÓÊ89W@¦ÜG©ã?þ0n&nª¿É¢ãj_D¿ÞÒý¾\G¿èQÒ?ÓT¦¿é°‡ÿ=¿ëoc/zA¿ïý…1,ȶUNASNone?ä1µpJüå?ÊÉa·™Î?ל•j7?ÊÉa·™Î?Ój=Œtå?È®‡°k Á?æJ÷a9ō?È®‡°k Á?çˆ]Ñ0M"?¯Ó']D?ÐïD]Ÿd×?¯Ó']D?Þ¸ÛQ'˜~?­	ß 
¸E?࣒Wl3Á?­	ß 
¸E?Èxõà€ ?Á/ŒwG4?éá‡ú_Ø?Á/ŒwG4?š8¯ÈW?«wş·ù?ï.:†ÊÆ?«wş·ù?Ë-sß(x?²?N'¶á?é=ô£5â?²?N'¶á?•'‹Š
¦?DÂä(ü~?ïSs£¡ì`?DÂä(ü~$MIXED4FGL J0712.0-6431?Þ Ì‰!ÓÀ6*¦óõ/ÂÀ;'24/²uÀ=ï4Ö¡b@§!,JŒ?ý8ø¤ÁëÈ?ÑUØInß?çï~U@Jâ|az?ùÜ÷&èw"¿îªi?ߓú?Ó߁w^¿È*è7¿ãÆ}'s¿ïÿ¤Á	?¨~¡½÷¿6UNASNone3FGL J0712.2-6436?éêìm¯Ž?Ã'åÜ,*?ÈTNIAÅü?Ã'åÜ,*?çä¸núgB?Åà'Á濽?Ð6"1{?Åà'Á濽?åwŒK}Vî?³íßصf¾?ÕçiR$?³íßصf¾?çÅύFz
?¬Š@o‹?Ðt`åsæ?¬Š@o‹?Úw	n547?Êޔð)?âÄ{Håeå?Êޔð)?Ê6ï;Ì?ǨÊþ°?érD1Œû?ǨÊþ°?ɽ°8þŠ?µÔu
£J«?鐽ÓñÀ]?µÔu
£J«?Ë¥¸`Ë?³^c$b?é'ß»çÍ?³^c$bMIXED4FGL J0712.8-5637¿íöÔBëj¥À3"µþT.UÀ:¢P0™û¿À<bg.'Å@ôê†ñ÷)@"dUêî ?ËHhbj?Öq"'›@x—Ü*7â?ÿ5Œu?æâ"Ÿg9¿Â'N¹Ìiû¿èϕÔèû¿ëf YžØ¿Û<-'ÅË¿ïþæZ<ŒxUNASNone?ïíø(ù¦þ?`›¤ªO?bÖí›Ò?`›¤ªO?ï«~?îNõ?ŽÙÈ4–ó?… oý
Ê?ŽÙÈ4–ó?ïIh}ÂÎ?‡'l82Wˆ?–ÞîØ4?‡'l82Wˆ?ïˆo}"b?rˆ˜°‡'?ä;'ø÷•?rˆ˜°‡'?ïÄ(¾:8?'ËnË19?}ük†ð6?'ËnË19?í¥KF­ìë?¶iæ/ ?²Õ¥ÊþŒ%?¶iæ/ ?ì"%x ?­Db¬Y?»^×¼??­Db¬Y?ëH'}=÷?¬ñx™<ÿ?ÂݶÄ&?¬ñx™<ÿAGN4FGL J0713.5-2555?ﱶmÀ Â	$lÀ:`öqÀ;ôó±³l@"®R
hô@éu½~â?ÂC| 7?•g'ߐô¯?ÖÑá^ª/i?ý¼&1$4?ïa‹€|<<¿Þà¾FL@¿è´÷Ãñ[ø¿èû9Ç¡ë¿Ð±©ûçl‹¿æD˜5kUNASNone?ïú\º³?8ˆGÈ>?Fƒ«³·?8ˆGÈ>?ïê
Ññ0?p–ï;PÕ?eõ.ò-ß?p–ï;PÕ?ïÛzYãK>?hŒ«c_½?rBÓ+7¢?hŒ«c_½?ïîÂO'±À?Fbýo\õi?a=°uO¦?Fbýo\õi?ïð?ö¶?Txží*?_€åUôÅ?Txží*?ï_\˜ ?ž±×s±ã?‹è(àÙP?ž±×s±ã?ï"O!«ï?†µÒ¾?Šì7œ &?†µÒ¾?ïte4¸‹?˜Vûcó?'sYllŠ¤?˜VûcóAGN4FGL J0713.8-4820c¿Âé@µ#tÀ0q+àŠðÀ:Ä©°ãÀ<G#çÆM@«<Û}"«@âÑk—þ?ÉâxÉhi?™OSǟ³±?Ñ&±dç`L?ý¨Tßd¿ÖX‹ýy½Ü¿ãCÿ~zÚ<¿ékEÞ±{¹¿Ûý¥|üªá¿êöÁBU&¿ïþ:bÒ]0UNASNone?ïõ÷ˆ.¯?K"<ÞOõ»?TðTÝ?K"<ÞOõ»?ïí‰×¯ª?o¹'|b?búvjHÕÓ?o¹'|b?ïË ¯Yì¨?pQqøðá?z/¨<\@5?pQqøðá?ïëɎ÷ «?H}T#Ψ?d6q)ە?H}T#Ψ?ïé75è®?d|¤›Ì>?fÈÊO•!¹?d|¤›Ì>?ï¿{ìñ–—?‡²=cê‰l?€!ËÙj:?‡²=cê‰l?ï¹B³Ñº?oR‡…?¯S
Cy?oR‡…?ï_|TNg?çç+²H?"ug6û'?çç+²H AGN4FGL J0715.7-1128?î˜I,;>½?´ÿ¾'ÜÈÀ9¼÷~0ˆÀ;`Πâc7@o!c'Å@¢Ž…i`í?Î7^¦~"j?Ú°km6d@@º°k?ꏳ`Xôþ¿Ü*«Ú佄¿¹ž+࿯¿èðCÊZ+Æ¿êN›n…êLžsóí£¿ç+ áCUNASNone?îR+¹lGÒ?¸ݓã_?ªÝDh_›ä?¸ݓã_?ÒV¨"TI??Ëu8•Œˆ~?æÔ«½ÕÛa?Ëu8•Œˆ~?ëޔÅC?¦$<¯º–Š?À…¯ëŽô?¦$<¯º–Š?ÖRÅòM?°"|x=×¼?äÖúp†Ù?°"|x=×¼?꣯¶Ö/;?ÄA]ãŠÿM?ÅqA$§C?ÄA]ãŠÿM?š¨åŸ©?«ýÓëOí?ï*¸Òç:"?«ýÓëOí?Ø.'Êb?¸¦«¶2ɯ?ãè±7xšÏ?¸¦«¶2ɯ?†[jŸBY?tgš#g7?漣Wþ;&?tgš#g7MIXED4FGL J0716.0-0826¿ïQ'bñðP?ù<¼~ ïÏÀ:$OTÑélÀ;¬ÓW*‰A@ç|\@?"Àh¡?Ð(Zý|˜?Ô)ù"Á ?ùb.þñG?ñrZ5*¯+?´Äúâ‰Í¿Óãº¥¿èq'>3Av¿é¢á ÁÁ¿ïøìˆ3@?ïÂpóˆ"yUNASNone?ïf½\õØ?«‡G?"'¨V?«‡G?êЬp¿c`?ÃÀ>BŸ¦"?ĽN=r?ÃÀ>BŸ¦"?íҝÓ~Ün?š-ؑAÙ?±kc›)?š-ؑAÙ?ëÞ
£›ií?¤ö›Â±u?À‡Éq'XL?¤ö›Â±u?î˜ÑYñ°S?§f|®ù¾x?¦rê`äúÊ?§f|®ù¾x?Ä?ò*Ì©´?Ê¢åÑ3A?êðuLՓ?Ê¢åÑ3A?åj9lˆ>}?·D%|û?Õ+&ïƒ?·D%|û?Ëôe(©©?¶ô%¾®æƒ?éæ½õՖ?¶ô%¾®æƒMIXED4FGL J0718.8-5004¿êï{¯½Œ,À0Z\å´$_À:͇
JܝÀ<…f?Ð@³â@0Ö­3ª?Ëq}Ü#×Ì?Ú~FïƒÜ@¬>/æx@ ¸=s¨ï?ï›ÞÒê¿ÒOZ±&~¿ÜŽèÑQ­¿äÞ!ž`RÑ¿éO"¡2O¿ðUNASNone3FGL J0718.9-5004?ëïÃT܃Ø?¸I <?À@ò¬ð¢?¸I <?íŠ*öE8'?³«s¹²ª?³®¨ND.ú?³«s¹²ª?ìùÊÿ˜&'?£ÍBÛ 8ë?¸1¨ˆ©F?£ÍBÛ 8ë?ítÔ¸Kþ?wÂ^}Ç?´YZ=9üŽ?wÂ^}Ç?åݳ<¶rK?Ã÷%Œ'±.?ÔD™†"j?Ã÷%Œ'±.?à!ª­GU?Ðį"<CŽ?ß¼ª¥ÛqU?Ðį"<CŽ?Ú6Qâm??¿eë5ä?âäòWÉ`?¿eë5ä?áõÜ•_<?±Áz7*mû?ÜGòÕAˆ?±Áz7*mûMIXED4FGL J0722.4-2650?³\Üp¸À¬	Þ¦%À:ƒsñidHÀ<D)ÿ®@\ó4ëo$?ÿ:¤þQª?Ð=;"G?á%K~ƒ"ž@aL¾´?þšBѶÁs¿ëqA@'m¿Ú‹2äôQ¿Ï4`¯Ã'¿åËDÂ&ք¿ïý¨¢K?¦«Qý΢eUNASNone3FGL J0722.2-2648?ï)q5ˆ‰?š¾Â¨Cœ?šÐܾŠÔ?š¾Â¨Cœ?îB ‹Ñ/?®‹³¾8(?«Õ÷F\«‰?®‹³¾8(?ì6ó4B?£" «=¨O?¾HgwÞ]ï?£" «=¨O?íydâÐÆ?•Ú(LqÀ?´4Øé†M?•Ú(LqÀ?êðŒ©e?Àæ¨ÑÆ?Ä=ÍË¥Zm?Àæ¨ÑÆ?ßóş†îq?ÒÌ¿á¬Ù?à0<ˆÇ?ÒÌ¿á¬Ù?â`M¾Qµ?½¡uõ¿N#?Û?eƃ\–?½¡uõ¿N#?့ô´®"?º­-Â}_ô?Üþ–¢ø?º­-Â}_ôMIXED4FGL J0722.7-2309c¿ÆëBS]öÀ:og—À9šñÎäÕÀ;LzÜ?0—@Cÿ‰7¢@y͛ÿ¥g?Ê»y'¾?ÓE‡~d	@	êºp©¶?üXùÁL'?Uª×¿å3éèwM¿èՉÕwõ¿ì;C½Äò
¿ð?ðUNASNone?î—à'ô‡?«2éy3Y?¦÷Ü-'?«2éy3Y?è­2R¸‰Ÿ?É)%¼Ü?ÍK6µم?É)%¼Ü?ì\6ÉY"‹?§bÃGÀ?½Iµ3[«?§bÃGÀ?ê…FT3o)?¨ááõ"ã?Åêæ¯2CZ?¨ááõ"ã?ëËZ
QVy?ÀáîXHý†?Àҗֺ¦?ÀáîXHý†?ÁÁCÆm&
?ÈôC‹gt%?돯d¶}?ÈôC‹gt%?á#©sÁ?¸"žåªk?ݸ­Áä}?¸"žåªk?¿.¿Iñ)'?¯eF(Hí†?ì(ÁÚÎ?¯eF(Hí† MIXED4FGL J0723.1-3048?ØY=iÔRÀp®SeâÀ:¬ä_‰PÀ<<v`¯m@@ÅIìˆ)@NŽ£œQÛ?À÷5Á'쯿˜šŸ˜·?Ü´O'…€?÷Q•"&h?î"gñ€á<¿ç[}Õ¿å÷ù1~'¿çŒþ«—¿Ú¡ûÁVÍ¿³+ooyŠ…UNASNone?ïû–@k!ƒ?>ŸÈÒ®÷?A¦ýq†Ön?>ŸÈÒ®÷?ïá}¢±ßû?xù"¯šl?n']9'\Û?xù"¯šl?ïæ';ßÞ?eS֒°ˆª?iëmð"?eS֒°ˆª?ï߯UB§š?SqWCÓP_?p(UdÛ~Æ?SqWCÓP_?ïõìÉÊíW?NÚÅޒ.{?T&lÕY ø?NÚÅޒ.{?ï\¡Ü窧?¦Ê'+ît?"kÄaRÝ?¦Ê'+ît?ïÖĆ='~?y¨Ò¦?t¼óÌ¥?y¨Ò¦?îï&I‰?ù}b ?¡ý˜Úrv?ù}b AGN4FGL J0724.8+3016?½æÍK@3öuy(àÊÀ;±™]3·½À<½`µL}‡@#nxY$È?ùÝ5µÄr‹?Ƕ÷xr¥¿¨ócå$?âEy¡¬'@šŽË·¿ïÿDÿ8"×?ïÿï0l¯¿æôpŸû2'¿Ñüf£".~¿ê•ïUÑ?áºæ ³iNUNASNone?ïþ¿¢í«?-–@ùî†?/Ô	RXàÑ?-–@ùî†?ïòk5"G±?\áN:%åË?[)•B¤lÀ?\áN:%åË?ï¾®S†¡?'"Y@ê} ?€T|ùŒ³¬?'"Y@ê} ?ïùú(zž?@NځU>?K¸|¯+9?@NځU>?ïýEÄ
B?7³¬œü'?5ÑÞçyôÕ?7³¬œü'?ïÇ ^k?,23ì(?|/ÐáÝÈ?,23ì(?ïÃÜþô_?ƒƒEÝîQê?~€ˆ·U?ƒƒEÝîQê?ïÝóÙ´šZ?lŽµŽ7}Õ?q'—5?lŽµŽ7}ÕAGN4FGL J0725.3-2550c?ã øBÇOàÀ†¤û¨'À9Íí'?2EÀ;c¡®;N@-8œ(À@Åôÿý²?æhàÿ‰¸{?äužö$à@
-«Þ7@È{"ZÃ?_î}!¿á¼üJÈü¿èÛrLM¶l¿ïün{Þ¿èÁÞ\AIv?хõB6Ü5UNASNone?ík™Þ
?Á§^Ô Ô?´§Wôzê?Á§^Ô Ô?êC©Sn?ŝœþ¼?Æñ[¦³¢H?ŝœþ¼?ëã-|Ã}¡?ªxV±p?ÀsJò	{?ªxV±p?ë¨<Š¨m¥?¥÷åÚXß<?Á_
Õ^Ij?¥÷åÚXß<?꾟û?ʳ"Þ¡_?Ń""?ʳ"Þ¡_?Æj<Ì[….?Ìé'¼2v?êepÌé´?Ìé'¼2v?ä2_´×Ÿ?µÜcãÕ'?×ó›@–PÂ?µÜcãÕ'?ÄD$®F`?¸p•HL&?êîöÔngù?¸p•HL& MIXED4FGL J0725.6-5008¿Ýô•Âä/"À.À'ÏR¹
À;/ìVÕÐÀ<"ՐÀ­@ ÃÉñ%F¶?ÞW> YQ?Þ%œSÞ$?ï‡ÁàŠ™Ì?ýC·zU0´@-'U°5½?éQS¿Å¨@?áµVÄ1ó˜¿ëh"ÞÒ2è¿Â2ÏJ«tã¿ÍGöµÿV¿ðUNASNone3FGL J0725.4-5007?ïôþ±Ã©Z?RC,ðaô?VœIòœP?RC,ðaô?ïï·è†‰?c¥¿l
?`H±Ð"¬?c¥¿l
?ïtØÓ|z‹?ˆ% (
Æ?'d啘•?ˆ% (
Æ?ïâò]Lƒ´?]Õùì÷Û?m
¢†!tž?]Õùì÷Û?ïש€#?y€žù8fR?t«žŒB"?y€žù8fR?ïÄ>@àù]?'øûŒ¥?}àßy…ш?'øûŒ¥?ïR˜}²)Ö?'Ò¨IƒÙH?•¬ðD"[Q?'Ò¨IƒÙH?ïâ¡÷GZï?mˆ`2@¬?m^…ÊÙ§?mˆ`2@¬AGN4FGL J0725.7-0549¿á`ґô@¼ŒÖ<¸À:$ÕϪ͟À<'¤ýzê'@ ·E¼wÀ?ü.;—…Ã#?Äãâ'§ä¶?Ã"?Zˆâ'@üäŒØ@s	¶Z?æÝÿŸ²ãB?í€FacGM?Öå±àHþ¿ÛOȶ«¿ÜìØ:¿¯¿äJè0-UNASNone3FGL J0725.7-0550?ïýÜvh‰?(3bè ö?1½ýXà?(3bè ö?ïÛ@å<I ?yxeëäät?r_IÎ+ý?yxeëäät?ïòå3\4?Xü»M+«w?Z5™ËˆÌ?Xü»M+«w?ïºãØÏ[ë?hDƒ)Ð?G	Êq7W?hDƒ)Ð?ï÷yRk ¤?M@"ìŸ?Q
ZÁJ˜??M@"ìŸ?îí•: v?ªªÙmB0?¡&¬T@ÐÔ?ªªÙmB0?ïÙö5ÑÉ?zvÞҜ?såÍæ¢?zvÞҜ?ïlÅ߆?ƒ¼Ñ*Í,?'g\ÞçÒC?ƒ¼Ñ*Í,AGN4FGL J0731.0+6607?å°¢Î@<ž"šVWûÀ;	µólÀ<°5ŽWF8@ß\>oQr@N˜™¿YG?Ï^ç–ýˆ?Ë
ïWúh?ûѽ¥è@$ÃÆ=ç?Õâø]I\??ì'©
Oå¿ß§ñ¶'!%¿àt`YÜë(¿ïÂXúìñ?ë6ElÛNUNASNone?ïϽ¸»P?ro¾qÙá?x!#‡ŠË?ro¾qÙá?mnŠn¦?‹}¢wvŸ"?€œ¤Re–?‹}¢wvŸ"?ïO»,nük?‡ÈuDè¡Æ?–šph¤­?‡ÈuDè¡Æ?ï(¨zÝì°?€ŸûRØ?šêð¤Bj?€ŸûRØ?¢·$š?‹àìHÐð?V×Gè"?‹àìHÐð?íÃ
غÛw?º&c#cn?±ç©:)$D?º&c#cn?íDŸ@;s7?£—"ƒ*?µÛýHF?£—"ƒ*?êÇ9LIQ$?¯R5<Xèþ?ÄãÎÚ»o?¯R5<XèþAGN4FGL J0731.5-1910c¿ÚÌ0X|¿È*VÀ¬'À9vf}ãZ®À;$(U{]@àšF<Ð@@sÀÁü?Ð`ÏM°Œû?Û¹1Å{@Ÿ€Á[ƒ@oå¤ßóÆ?´¬˜¿â·Í⠜¿éHL՛¨h¿ìÃ+c[¿ïè¶!å'ü?ï£êUsÐUNASNone3FGL J0731.7-1914c?î:šg
Äþ?»ßÌÕliÇ?¬VYÿ—?»ßÌÕliÇ?ë&|~ß6º?ñ­$L!?Ãfƒ%?ñ­$L!?즌èlv²?¢Ê•{WS?ºË˜¼œJp?¢Ê•{WS?í`˜]HI_?š®…[k'ý?´û=™œ	?š®…[k'ý?ëKÖbwÄ]?ÁsMµn¯?ÂЦv î?ÁsMµn¯?Âz1c>-?ɹ]}Öè?ë~as§0u?ɹ]}Öè?ß±¥¥?·ÉZ`"¾?à'-1w­r?·ÉZ`"¾?ѕöl-z¸?»5	ˆP,?ç5ÉéB¤?»5	ˆP,!MIXED4FGL J0734.3-4448?ïìY~Ò=À'ƒÌòŒyöÀ;ÔÈ("À<bZ¬ôÀ1@ Z¥@ð@>GÜ7£Û?ÃÍí^<Ì9¿Ÿ\1%´;ÿ?ÝC]÷)?ÿÈ¥Ó¹¥ÿ¿¼ șڿá \a)惿éQÓÂ_`Ž¿ÞÀúôÓQ¿á]Õh|Á¿Ö…Ôàík(UNASNone?ïýEü'r?+Ñ@ñ9µµ?7Uπp	X?+Ñ@ñ9µµ?ïñ"C4÷È?_"À!¤?\÷yðÆ?_"À!¤?ïñéJmÊ?Reç-}¿?\-koýûV?Reç-}¿?ïö -»Ò?7I!Ç<'?R¿¤Àö*?7I!Ç<'?ï÷4œaA†?LP€BYÅb?Q–ÇTŽ?LP€BYÅb?ïÆ<Y™ñ¦?ŽÅâNž†"?|áÓD59?ŽÅâNž†"?ïŸ[?g¥ýèã
?`xJH1tÓ?g¥ýèã
?ï´]ǨÂú?sÑR¿Ø*?'èŽÏA"?sÑR¿Ø*AGN4FGL J0736.9-3231¿ÅÆ…ß(ÀL™Â´EÀ9RyaíÎÀ;'¦éä4È@ˏ¼ÈÉ@$§š
\à?ºürùO7?ÕÒýhv@¦¢‹°£@—Ž§x*?ïÿñ_{'¿Ú;ô¢Ô«¾¿åÊZâN¿+¿ê÷']gå¿ïÿíPÐÓ?ïñÂjÉ"UNASNone3FGL J0737.2-3233?ákJz¼M'?ˇø(èy?Ý)k
‡dÛ?ˇø(èy?æO þ¬‡¢?Ë@VÙDn?Ó`¾¦ð½?Ë@VÙDn?äøÃr}m`?²U»Ø»?Öy%??²U»Ø»?éä1Â3°u?¨ù€2`?Èo8÷1>*?¨ù€2`?¼°Æ7:e?½pGÑ$ö/?ìiç=³?½pGÑ$ö/?¸ã¶¬ã?€sdÈùÑ?ì㞉S·s?€sdÈùÑ?ɓԾ]É4?°›D0qçî?é›
Ðh³?°›D0qçî?Áë5—?¯Xh¹â@P?똻E:òš?¯Xh¹â@PMIXED4FGL J0737.4+6535?ïH«Ú'Ã@=@W:yx'À;TûwCÀ<Û:aû›@ Ÿï 3Ò@Ðh˜oÍî?¾¥õÝè(¿±Œ,ž™ˆ¨?ôn$ É8Ä@‡ó]ZN*?ïì³I¬¿ÒZž\!¿æø'}sHL¿á˜çBsB¿àØÏo>|=¿Öј
¨_/UNASNone?ïþ÷÷óÂ?‡€hFO? €~UŒè?‡€hFO?ïô±V¾l|?VäR·ŸIu?VRÇß8p?VäR·ŸIu?ïø¥ˆ1ç?OîOX~‹D?Miݾh¹?OîOX~‹D?ï÷µoIJ2?3Ž
öÊÁF?P•!€©kÈ?3Ž
öÊÁF?ïþ€~‰?! "™
V)?'þ^m¡š?! "™
V)?ïÎßeoŠ@?{EN6™m?xM8l«î?{EN6™m?ïúì4á?SÏYÛBÐB?G—¯¯1àá?SÏYÛBÐB?ïÒi4T£ú?fC'[Cƒ?vËeå|7?fC'[CƒAGN4FGL J0737.7-8047¿æ®îüˆ¸À8îÉâ6Á]À;mðwÌÀÀ<®rØœ@"E…sª?ûêՖŸê?˹®øP‰/? 33"'K?֓7_'·¨@–Æ4WK¿ïéZ¢
¢?ïödá+(£?êàöðŒÅv¿ßýS]?á¿ËA×e×ö!¿ä?y'"UNASNone?ïÿrJ	7?÷a †.Ö?¶µdû0»?÷a †.Ö?ïö]'|?WP0løÝg?SãE"£y&?WP0løÝg?ïõG[D…|?TLr÷ÿ¸€?UqIp§R?TLr÷ÿ¸€?ïü'Ò­·^?,À#Œs[?;éjÊXJÎ?,À#Œs[?ïÿxZ§ì?
TUùa"?ô¤²Õ±M?
TUùa"?ïÛMõg†Þ?{Ý–"£¼?rYjy Í?{Ý–"£¼?ïñíg‹ª?h¬gBׅ€?\%Û©Úê}?h¬gBׅ€?ïù?
m7?D|9¾¶)ƒ?K¯G£I3?D|9¾¶)ƒAGN4FGL J0738.6+1311?ÛW5*#Á@0TC^úa[À:¡1¦¿óÀ<TÇ$íS@wð¶6y@È7 þ}I?ÀŸ9Q´~¿šÛ"CwÆ?Ô6߇Ï@¸¹jyN¿¥´)gØV¿éyô'ô;§¿ç)GŒ†‹ ¿ëËì't¹æ¿¹` Ò¿ç†lªMFUNASNone3FGL J0739.8+1312?ïþýC­+?™ÉªánQ? +Ñø ~ñ?™ÉªánQ?ïó0¹'ËÃ?]C´C–¾*?Yžhð™°?]C´C–¾*?ïñy"Ñ5'?ZzÇóÿS£?]ö`T‹–?ZzÇóÿS£?ïÿ
MЇ0?ÒË1[!Ê?¶KKJ»t?ÒË1[!Ê?ïüѵcÜ?:Ÿþû5s?9rT\ˆ©Ö?:Ÿþû5s?ïÀÀs'áÙ?†ûc§Þð€?ŸÆ9ÎÃs?†ûc§Þð€?ïèܧ­¥â?o)¢ð!¿?g#Xàýß?o)¢ð!¿?ïø^	d¦?Edü&èÄÛ?N‡ÙK!^1?Edü&èÄÛAGN4FGL J0739.6-4530?áŸF]Ì'ÐÀ&~gµñ¾õÀ:€ÄK"À<ùqp…¤@üoò2b@ùI¥e·?Ж@.l?Ê"hܸ?û‹Jì\t?ð<x{í¿èIg–Øõ¿ßܔÀìĺ¿æ¢þ)q¿äç½~{0"¿ïÿ}ž¼C=¿ïÿ·¥ôïUNASNone?ï`´9X3?°îö«$?"éxßLǨ?°îö«$?í½OWðƖ?³vݞÂ}‡?²…@ç¾Ð?³vݞÂ}‡?î†×ïî\?™¬ëÌeu…?§'ŽÃ"Ï6?™¬ëÌeu…?íà­u!G×?'UçòU
?°ú"X?›Ç?'UçòU
?îß`¡'›Ú?¦ ø£3Y?¢	õêUÞT?¦ ø£3Y?â*4™º¦°?Ñ`ò)ŽÕ×?Û«–ÌŠ²¡?Ñ`ò)ŽÕ×?ê(âªã!?±æ0üGŒ?Ç»\uTs}?±æ0üGŒ?ßfԔ†#4?¼óÞg1›?àL•µ¼îf?¼óÞg1›MIXED4FGL J0741.0-5226?ٟ
Š{!<À,Xépq'#À;wï‡â·ñÀ<Œ¬&dØ@#E†•…ã¯?üCïÉQJ?Èùƒ<Ù¥¿±P;ל‰Ž?êÀSAÆsí@¸(Üî'¿ÌH…ªÏL¿ï-¸À%t"¿ÔM›iR¿ßWçÝõ>0¿åÃcÍ.ò\?´å€ÝNêUNASNone3FGL J0740.6-5230?ïÿ›•Œ¤>ýgÓ¬?	Œ52«>ýgÓ¬?ïôèßÄî?Z6Úå
?V/î-8S?Z6Úå
?ïú£ˆ–ù?6"³zõ/ü?EqÜэD"?6"³zõ/ü?ïýߛÓÒó?#Í'qƒ	Æ?1¼K?#Í'qƒ	Æ?ïÿ±›ÃëR>üµaÍ#±V?™Cþ6€>üµaÍ#±V?ïÖ'8{?Ší¬†>?tìcôy—?Ší¬†>?ïûÖÊ|-?XRé?*U?@¤×4ö6¤?XRé?*U?ïõ³íu?Qàâ©èý?T™Ú›¶?Qàâ©èýAGN4FGL J0743.2+4034¿ïmnK@:Yæ%cgÀ:ÎÓU}
À<~Güó@ÙJ¡!@|âąÖn?ʔ]Úü_?¸hšÉŽò?Ù‰@¢ŸÒå?íáH2ž¹¿ëzá³
Þæ¿î
# îø¿×,RÙÁ§Ö¿ïÿT©¥€X?ïÝe¡D‰UNASNone?ïúìÝäLE?H©±?DL‰|½
?H©±?ïê9;­L¡?uRל>N—?eÆÄ8–Vé?uRל>N—?ï­	ÖmŠr?—x{•ŽN?"½Šdc~?—x{•ŽN?ïð¯ç¨Š?Ppu"1ÔG?^ 0N¶Î1?Ppu"1ÔG?ïúªT
.£?KxðÆj?EV¯y['£?KxðÆj?ïsfÃÒ?¡è–"Ef?'"=bu»Ð?¡è–"Ef?ï°#w"Ä?";#‹Ûþ?ƒ÷"
ìÃ?";#‹Ûþ?ï(d7.ŒÓ?"'²`0Ç?šóyO-´?"'²`0ÇAGN4FGL J0744.4-1403?â^íð>Q@‹"ÞQZÀ:Qo­7PÀ;å‰bÙ@̀;¤›Ö@ÖwÁ½o?А^\¶#?×>š?‡@T¯ÕEAS?ôBñ—1Š?ï³ÃçJýT¿æÕ `]7é¿éº øžï¿ëÇC‹p+¿ã%áæåR¿ïÿÕ¾
iUNASNone?ï""©£'?±*ð\žl?Žþ·U—6=?±*ð\žl?è‰/öà?ɖ*Y}—?ÍÛ@$³Œ?ɖ*Y}—?îf¤Ç¢?˜.ê·	?®	•²²®ä?˜.ê·	?ì
N¸tÑ?¡ùXÉAR?¿­Š<Yx?¡ùXÉAR?ï:Ê¥]Ñ?¢}§nÆ®?˜½&°{¯å?¢}§nÆ®?ÁZ"ß½?Èe¸Ì9Ôã?ë©wH>½?Èe¸Ì9Ôã?çÁžx¯?»FNÃÝdõ?Ð}øáÈ?»FNÃÝdõ?ÐE!Nі­?»$TøC·Õ?çÝoX—4©?»$TøC·ÕMIXED4FGL J0744.9-4028¿ï×җ"WÀþô›»³À:mµWeA£À<f
w"@š—ƒê°¸?ü˺bfý?ɪ`;Tþ?ãÄZ7ƒúÌ@ßbц@X—²Ž³?ïz͑êØ¿Òê?yg ?ÂâÙ(¦¿äÆhÏÍ2M¿ëFz£4M¿àƒ ˆ÷
UNASNone3FGL J0744.8-4028?ãúƒLXѱ?É~åŽq®?Ø
ùgN\ž?É~åŽq®?éòˆ"tÒÌ?¦î§-'?È5Ý®,´Ð?¦î§-'?âÒljۥG?³ÜéÇѲ²?ÚZpìHµs?³ÜéÇѲ²?é†JKAŒ?¤=ìÇ)yë?ˑæÖÒùÑ?¤=ìÇ)yë?ÄÁXÐP»?Ĭ+*ô?êûÏ©ËëÑ?Ĭ+*ô?ÑÛ«"öO?Îp†®cë?ç*qî"Ø?Îp†®cë?»«ÉûiÌ?¥EV¹Y¯G?쟪†À'Ç?¥EV¹Y¯G?×ÑÊ\üÚ?¶åüŠî?äÑñ"?¶åüŠîMIXED4FGL J0746.5-4113¿ã}É6Í
À 6‰Å!ÞÀ:«°ÿç¬À<IP«éþ@8ñÁ"õx@›²ãízÂ?ÊÄ3êé?µ•þk?ì«Ð¾Hûq@^ðTf^¯?ïþÖ~z¿ì@9
ãˆÑ¿ØOr"¿ßó«z=¿ç›#§¤õ¿âà¥Ç¥EŸUNASNone?ïüS&‡m?>ܺ׎€?=fÌÓÒ?>ܺ׎€?ïîÄà*ˆÑ?e8{»	®?a;¡=n?e8{»	®?ïìͽQs?l¨ÌÌ{¶?c2Bé¥ÈÁ?l¨ÌÌ{¶?ï蚂;Õ?GáÀCŸ÷?ge}—S"?GáÀCŸ÷?ïüáG>?Edl}??Ïà®N-?Edl}?ï·:Ïè=Ê?'ÙXV?'1L
Às?'ÙXV?ïÕâÅ?}pêŠ=?u@úuýµ?}pêŠ=?ï‰þ_Û¡–?u»g!ß½,?€hfn‡?u»g!ß½,AGN4FGL J0747.2-0736?ïÿí'ò/ª@!…–À:Õ¹Nè›À<MÓÔ(
á@ Œ-·c?ÿÚÇ犾5?ÏÌçå,0?ªå Å®‡?à(È
Æ, @Rn6êM¿Ùù–#ÃS§?×ƺCÞ&;¿á'àb*íi¿ÙEÉ7ìÖX¿çÂb¿¤?h50ìåy UNASNone3FGL J0747.4-0734?ïýp7íÏs?(-Oa<?4~>{'g?(-Oa<?ïåÚÍ
ï?qíTS9?j%2·àÉ?qíTS9?ïð%X1Î?Z²Gåð¨Ö?_Ç´éçôË?Z²Gåð¨Ö?ïéV¿:¤'?JPY:­Ã?f©@–¡)I?JPY:­Ã?ïüÚ¤ëv?7z¼h* Þ?;ñ)َ7?7z¼h* Þ?ïFH0ÆFv?¡ö§GÊGv?—6ùãǕI?¡ö§GÊGv?ïä¼®­¹?vë/gı?kCQ.Šóµ?vë/gı?ï --Eð?wºî3?Œ·ôª_°,?wºî3AGN4FGL J0749.8-4420?å±/™ô;À"3󾩛À;9
£3vÀ<µ"6Æf@©ûv®] @RB<»r1?Ò娛•\?äÅýƒxñ@`ÔV.?òasÝó:Ë¿à†øaûó?UAª33¢ß¿»»Ñ«Xß¿è9']e5å¿ëUÛN¿ïÿýawUNASNone?îÝvF?³n¢M†ì?¯ÏÎýݨ?³n¢M†ì?â¦OèÉ?ÌzAî¤?Ú³Í`à.m?ÌzAî¤?ìðe$5Ù?¡äv'˧°?¸|Öà	0?¡äv'˧°?ãcêͶ#5?«úXq?Ù8*d"¹—?«úXq?ê«ðT¢Ø?Ày·?á†?ÅP>­vž?Ày·?á†?ÀÓmì¨Æn?Ä»¯í_?ëË$"ÕÎd?Ä»¯í_?åW0lO¬?¹#>ø¨¼?ÕQŸÑ'`¨?¹#>ø¨¼?¹Ÿ½1@?ž,íV¬ b?ìÌ_ÜØ?ž,íV¬ bMIXED4FGL J0750.0+7140?âff˜T9@>>A€ÓÏöÀ;'u¸êÀ<^£ƒ'gM@ia ƒî@™æáK	?ÂZ	‹Å¿Á0'B]¼?ð֑§\л@QPiÏÒ¿æ{¼n°·Ã¿çýՃT´¿éØ·¡Â]¿ä´>Kë¿ïüž…¿ïï,"¹ºUNASNone?ï÷êoŸõÿ?Q9–­sô?P+!&Ϙ?Q9–­sô?ïàL/z?~l1fkÅ?o³û^tnV?~l1fkÅ?ﻗ>[Áƒ?}+}ŽÎrë?0f§åD?}+}ŽÎrë?ïØî…H¶?]ma坳?sˆ½Yäa7?]ma坳?ïÑžbMŸ?…¯¥/àÿp?w~°Û7È;?…¯¥/àÿp?ï6¤¹!8#?¥·ïÖH=à?™+hݐɤ?¥·ïÖH=à?ï©|#¾ ?‰'GàËÉ?… ÷=?‰'GàËÉ?í7n¨C?¨r//þ¼?·^G½Ô˜e?¨r//þ¼AGN4FGL J0750.5-7519?¸ti"ô7XÀ6ŽØ
±À;!n
#ÔñÀ<wñ8¼ßð@–'âòþæ@«Âßä?ÓʤzHF?ÛÞ¨éϒ@}€Ú…ó@Œ T‰D7¿ïÿR@>´q?ïû¾½?'?ì"}Š¿èîê.¤¿á‰ ]9–¿ïüö@
·#UNASNone?ï÷ÎU‹¢?JxFÀA×S?PcV3aÚý?JxFÀA×S?ïìRðNv?dÞVU­Ì£?c­Ê¥¹Ž?dÞVU­Ì£?ï[öPÝEÉ?ŠÙi·i?"5ë6~É?ŠÙi·i?ï° ;´·?oo‹™ŸÐ?ƒ÷ñº™­?oo‹™ŸÐ?ïð:o"¸?^Î|J?_Šå#–?@?^Î|J?ïÂP«zRé?ƒþb¾]•ª?~תN…7¥?ƒþb¾]•ª?î½pç|Y ?šB	k·Ô°?¤(ñ‰ò<?šB	k·Ô°?îÜ3s?"Õ(n'¶ª?¢>œÆ:Zœ?"Õ(n'¶ªAGN4FGL J0752.0-2931?禘ÙçM¾¿ômY4N¼&À:¼&Œ[ÃÀ;èH÷À–^@]6fïM@]<9Aj?͐½'h?æêúêíID@^Íñ?ø~…—<¿Øy|ӆ¿µjF€þÿ5¿àùI—ù†i¿ë÷2ú(P¿ð?ðUNASNone?Ü]!n9Ä?Ð]ðÙU?áüÑoHã?Ð]ðÙU?Ð0'©ÆŸ?ÄÙ<'Ÿ½?ççìu+±?ÄÙ<'Ÿ½?ÞëÈÅÃ?³}CÒC­u?àŠrõŸ?³}CÒC­u?ÛÄGƒ
?µÂÌ»"r?â~Ü8>z?µÂÌ»"r?¢CØ.k(?´:xÕ\pø?îÛÇâŠ×½?´:xÕ\pø?"Úɀ5F?¥{|Ÿ¤$×?ïg	)}–?¥{|Ÿ¤$×?µY…8Rq?£FšÏ;Ìf?íTÞo='?£FšÏ;Ìf?–YPùùê?ˆïX0•?ïM5x÷Á?ˆïX0•PSR4FGL J0753.1-2624c¿Ï€¸L7;+?á!l—¥À:ŸËz½5€À;÷ÏdVÁ®@ùáxÖU@1ìVuX?؀ÌÄjÁ?îܘQšýG@4' ÷@f"ÄB¿ïÿñò÷?ïÿ@Aä{ë¿â5¯^ý¼Y¿íLE¾P2G¿ïÿýaw¿‹4J_t¯ªUNASNone?èWÄ.?Î%
F ´|?ώ ïE¿õ?Î%
F ´|?äüþz2º×?̉ÁÚD?ÖšŠR?̉ÁÚD?éC$ÄýÂÛ?°!͈&?Êólìô"?°!͈&?æ«®>Â2•?°µ{s+?Ò¨£'{šÖ?°µ{s+?ÜÕd‹ð—?Ó»Cɔš=?á•Móº´?Ó»Cɔš=?¶O'ÇŸô?ÁãWà‰©?í6§E‡Q?ÁãWà‰©?Ü/¦Ã›@?À\Ñqøú?áè,ž2t`?À\Ñqøú?À9XÓÎD?¨¨9(™?ëñ©Ëz¯?¨¨9(™$MIXED4FGL J0754.9-3953¿ë8'Kج»À?Ë~3ÓÀ:¢rúÉÀ<ÄxCÞ|"@Ž}á,U@?Qi›?ÌEú
G¬'?ïþ¡€Ã´Ë@öÇê弈@WzK˅z¿ïÿú@ùDz?ïþ¯¾3G?æiªK¿Û©q="ðÀ¿ð?íáŸËŒÜUNASNone?¢™¨u9ú?·!¡x¾¶<?îÖexñ'?·!¡x¾¶<?Îwq4?řXÞ(?èz9¢8#³?řXÞ(?ÒC!'ÌÌ?±óœ¥í®Ò?æðÞo6™š?±óœ¥í®Ò?Äî
×kُ?®&èØ3AÓ?êÄ}J%	œ?®&èØ3AÓ?µœu{‰£?ɺ¨ÕC5V?íLqPWäÌ?ɺ¨ÕC5V?¤.²Úƒ$Õ?°ô»yŒ_ª?î½ҎÇr?°ô»yŒ_ª?ÀáèÚ-*?©uÅØP‰f?ëDžøIt¶?©uÅØP‰f?ŠôŽ¾¼lA?…%1ýN?ï"-ÅÌ¿?…%1ýNPSR4FGL J0755.6+1855?Ð%4õú\@6_ºº{'qÀ;]K´3xÓÀ<¡ÊVÐÇ-@´¦M@"Åyò4e?ОÖd¦à?yT¿"~ÕÕ?°¥ô›ÈÈÜ@~ù ?ïíL~Þ­J¿Þÿ<÷S½¿é­Wâ1»¿»uøÀ·¼¿äd¶Ê,¿ðUNASNone?ïýÚ¤"aØ?%ïÏ?aó?1*Ýùæó¤?%ïÏ?aó?ïôÆ"ä†}?XW	ÖàMe?Vsº
ø"?XW	ÖàMe?ïðìß[?YM~-Åo'?^&A¥Pì?YM~-Åo'?ïüÔ²¹?#eëÔ˞??i\º/Ô?#eëÔ˞?ïüûØöH>?7a™`®Ry?8!9í[E?7a™`®Ry?ïÒÓ>"qç?{"ÔA€à?v–`Óú'?{"ÔA€à?ïå7ÅǨ~?tsa6
?jÈ:*™Ò?tsa6
?ïðvA%¸?PNBpLu"?_|îïà™?PNBpLu"AGN4FGL J0755.9-0515?àêÏ´³¦`@''´·,RÀ:‹kÙlîÀ<³'àÚ@O—íÇï@ðù'7}E?¿µ2&mÒì?¨VL_KŒh?ãmjñ¢?ôäŠ$[ª¿Ïl?XÛci¿ê-Ôï°ýc¿ët·AË&"¿äü¦¯+Ò¿ïôèà(Ê$¿à†HNMjíUNASNone?ïИÛrpÐ?Ž*'5<?w³'RvD(?Ž*'5<?ï&¼Aå'·?¤¦@æ·õô?›(wÁ£;?¤¦@æ·õô?ï=ÁrŒË'?­îoœ¶~?˜Gѥχè?­îoœ¶~?ïcƒï˜?†xO2rb?œ3ƒÓû
?†xO2rb?ïNfŒÉI?™tœij˜H?–3.jF{Ø?™tœij˜H?èYµ³"#8?ÏÁ¶)ƒmD?Ι)3ws!?ÏÁ¶)ƒmD?î¦mP,W?šË{‹ä?¥™.Nl֊?šË{‹ä?æŸsŒ$ø?»uAn?ÒÁç¶Ð?»uAnAGN4FGL J0757.9+7304¿ì_)ßU@>¯½¯ljÀ;Ï1_œÉÀ='òH‡XN@ šj$"?ûÁý¶y¤1?Ôp†yÇ?Îø" 5ª‡?÷*ÑJ
M@°sAI?혬3Ð%¿êVg€AÙ¿¿Ñ
7öçRŠ¿àëL4"†¿Ñ`Îvðø%¿ïÿî,˜å?UNASNone?ïù$Âé/j?I775EÅ?KlóbÄþã?I775EÅ?ïôš/°`Ÿ?Wt
§ë?VË AÉb?Wt
§ë?ï·Mpe¯?†:(E?',£Ú·²d?†:(E?ïõ€ªV͏?:ÉóxÞ0k?TþªéðÃ{?:ÉóxÞ0k?ïúÒI
?DɚägÈ?D¶Ü/tA…?DɚägÈ?ïÎØßÄe?zÊIF??x"7:"Ô?zÊIF??擄éÂPó?ˆ(hmÁhY?†ÓŖJû>?ˆ(hmÁhY?ïÛ¬•"?cÊF¬‡<?r)µ‰ éò?cÊF¬‡<AGN4FGL J0757.9-1514¿ÂrQ²‹i;@ë¹]"?•À:?eóSIÀ;Üèi
…•@T'ÊtX@ÎíEé]?ÌɞÄüžÍ?ÚX™Ÿ"ðp@
2Väé#E@w5Êè2?ïû™3BL¬¿áŸ
='¿é¾kÀÃT(¿îÔÚbaŸ¿ïrô^Œ'k¿ÐÚáŸÌUNASNone?ïbR—?˜4NÉä&?ale£,ÉA?˜4NÉä&?ìœÒ¯B€â?¸
êApŒ?»j…ëøó?¸
êApŒ?î…hýšu?–8X¿A=?§©p)ÈK??–8X¿A=?ì¶`UÄòR?˜Sy‡|÷Ò?ºLýQØmr?˜Sy‡|÷Ò?ﵓ‰?'çRurç·?'›³0LÜ?'çRurç·?Öè£_¢G?Ó´×]I‡3?䋮Py®Ü?Ó´×]I‡3?êsOá?¯Ò囔Š?ǟÆ2Ð}?¯Ò囔Š?ϝ)Ft?²‹Ë"0"s?è8µ®x#?²‹Ë"0"sMIXED4FGL J0758.8-1450?·£Ôz˜@sÞ¤e¥vÀ9éɼw4À<O‹À@Y{SJ?ý–ç½éÚû?ÉÁžÛÍƝ?â¶ÝÂhoÖ@Ÿ=áâއ@rÅë‡"?ßcøb|ÌÚ?ïàuöý!ÿ¿Æ:'v_'Ç¿äÕub'¬¿î"0Akˆ¿ïÿŝƒ‰UNASNone3FGL J0758.6-1451?ÁÚ×Òdf?Ä ôB	î?ë¹ÉJfæ?Ä ôB	î?¿QF]vA•?¹8sþ+Hì?ì×4Q7Í?¹8sþ+Hì?ÎÙ¨tË%z?¯¦V…xã?èI•âÍ6¡?¯¦V…xã?Ì8Íb/0U?«l16ÆË?èņ̃t3ë?«l16ÆË?¹"¼ÑÊ;?Çëï8Û?ìÍheïóî?Çëï8Û?í—E÷óü?"ú[4àۘ?ïx"F: ?"ú[4àۘ?¬(EÔ¬‡`?š÷¤
kÞ?î={¢§y?š÷¤
kÞ?"|5ã‡f?Èw˜öŒ?ï\î‡Ý…?Èw˜öŒPSR4FGL J0800.1-5531?áúÜÔúHÀ*@!ÀD(NÀ:Ìá*?À<ªGfÆÞ@ï°oÉçj@ÁÅg}¾?ÉÄ
'?–%"›ìÁ?ÑXŽß#@ÓÝ¿¹>?ï"¸Ç\J"¿â@!X?\¿ê
…/J¿æBM'iҿדrãø7Š¿ïÿ'ö֌UNASNone?ïûŸÒ)[?@šÕíã?A€¶IëOŽ?@šÕíã?ïòÉîöî3?\|"æ©?Zl!Çì	s?\|"æ©?ïÞw,Þ?mͬMªÈ‹?pÄi¦2Á`?mͬMªÈ‹?ïú´åá÷?,÷¸UíØk?E,i9HÊ-?,÷¸UíØk?ïóM·eSä?X³ôŸàÁ²?YdûžÈ?X³ôŸàÁ²?ïЉö¨,?‹"ÌiêCD?wüºëî¹þ?‹"ÌiêCD?ï¢mëÀØÎ?‡9Ð2?‡d…\¥?‡9Ð2?ï×&p4Îò?g~W
¶7?tlÇÏ?g~W
¶7AGN4FGL J0800.5+3715?Ù{Ázf×@='à°«À;¶–ʞÀ=jïVd£@Q±; è@¤+eßWê?֖©ÁÍ?ïþh@0FÅ@
ˆ¹w…s@dCðš²H¿éŸù8¿å";‹ÇI¿ÈE/‡­¿çTÁ£Mø¿ìrô´rbô¿ïÿ»×²UNASNone?íyK]t?¹½•Ñ|Ρ?´5¥‰ÖÜ?¹½•Ñ|Ρ?íyƒ›=^?¶×(.=G?´3çaS–?¶×(.=G?í,iÿŠ?¡²¦ÔP?¶œ·Ÿ'ÈÓ?¡²¦ÔP?éðLâÞ?¯2î-´]?ËÜ>Ïôt‡?¯2î-´]?êh½½ ˜?ÉYÁ6L ?Æ]	}Ì?ÉYÁ6L ?ä!^s†¾?Ð^í•Lá?×½CÇò"?Ð^í•Lá?ç?îûÔTß?¸¶‡D$f?р"WVB?¸¶‡D$f?Ó#þZlÑ?¸Ÿ'5ï"0?ænÒÉø?¸Ÿ'5ï"0MIXED4FGL J0800.7-1059¿ªþØÙ7£·@#ú£iüóÜÀ:Qû]ÙÏëÀ<9¬üLí@×Õë™"@ŸNìő?Æ	[ˆçÅ¢?ÅAòé—ï?ý'-K6?ü/š.êÏ¿ï²LîÆÙ?ïÇìÞe%Ÿ¿åÏ/!}¿åNžsž¿ïö§ý	«z¿ï+þ¶~ØUNASNone?ïÐÓ¸àlù?xÒ¦ˆné¸?w–#tü´?xÒ¦ˆné¸?î{º(/t?®gLñC{_?¨D]}¿A?®gLñC{_?ïU/;Ìú?ˆKéÞ6žÑ?•Zœ¦`Ê?ˆKéÞ6žÑ?îJŽ]j-?'d¡¡B2ê?®›Wá+*?'d¡¡B2ê?î@‡#ö?«pèí·‰?«÷á7|"?«pèí·‰?çWúƒ!?ÏèÇR, ?ÑPÌøý¾?ÏèÇR, ?í€Ï뇚?¦'ì?·ÓùYè¯?¦'ì?ä"f(uax?½ƒù‡J?Ö×3¯=?½ƒù‡JAGN4FGL J0800.9+0733?풼È?@Õ@2ÜJ@•òEÀ;~™Pž~À<éö\é@ Ž¨‹úʌ?ö½õ<ó¦?ÖHì'õ"@?げ©@ûA3¦ö?ö~ÌôºÒy?åè阵n¿ïÏYÚféC?ïÿÊ»z"ò¿•Ã0}¢¿ãÍé,~ä¿ïïá9k[™UNASNone?ïÅ寚À?zú˜½qª-?}
}¢³?Ó?zú˜½qª-?ìÕC'¥{?Ák¿ª%'?¿aUãêÔ'?Ák¿ª%'?ï ?"5•t?'"ÁŽ6VW?›ø|¼íp?'"ÁŽ6VW?ë›o¿;Ñ?¦Ï"X±öF?Á"¦A½?¦Ï"X±öF?ïµHaÌ+p?ƒ6!l¼·Æ?'­çŠj?ƒ6!l¼·Æ?âÁrŽñRœ?ÔWœnF?Ú}âZÉ?ÔWœnF?î|OÉìȖ?Ÿ c1Y'Ž?¨;]ÃÚª?Ÿ c1Y'Ž?å s·±¡?Áçº)î!A?Õ¿ؐœ½?Áçº)î!AAGN4FGL J0801.3-0617?ê–zrY[2@(èä¸{ÜðÀ:ŠS±WüÀ<s'È@ùº=S³@ ƒn—?ĝwI¸…Ã?œAí¤ø?Ö–­V?ü»%_5?ê?'—•¿±¥Ku쎿í3Ðçå¿Ë—¡ò®‰¿î#f!/a¿ïü]°	sUNASNone3FGL J0805.0-0622?ïÞ=âÛú4?jm¢û$?pá}e>E?jm¢û$?ïÃ3ófXh?†BN€¬èË?~fQ£?Æ?†BN€¬èË?ïf©Æýß?‰5㼨gh?"*Ç"²'?‰5㼨gh?yçUB?my€_p?ˆ'¡—X»r?my€_p?ï1çãËä<?–·ší?™Ã~u?–·ší?îÓ^'5?®tA[Å®?¢Êڟð·?®tA[Å®?îâJìýÂ?–t±è är?¡ÛQ.wµå?–t±è är?íi:ºȬ? kÄc
«?´¶*/§®? kÄc
«AGN4FGL J0802.1-5612?ï+ñ-‡Ö+À*kQœIwÀ9ÑÈDŽŽpÀ<Wí|o½'@
¤þ&¶ù?ÿ¡Å'U°6?À]¨½#ž?èMàÞ|¢"@#sÈ:–ÔÃ?üüo'ôn¿éÉ9d¥œ?Ðû‡n…D¿Õ´`$-ó¿ê$ŸANSö¿ïÿýç!é?èAôl#UNASNone3FGL J0802.3-5610?"ñu¯¡Ç$?³—íùÁm5?ïXtRY¶w?³—íùÁm5?Ã=Þ»jWj?À‡1Y‹¯?ë0ˆQ%j%?À‡1Y‹¯?Á÷¸ék?©='ƒf›?ë'Å¥;8?©='ƒf›?¬ñ·£%ü—?›«?€ÀÒ?î0䅿áÇ?›«?€ÀÒ?šGkÊ4‰M?ÀÌ»€°OÐ?ï-Ä¡… f?ÀÌ»€°OÐ?¤\täÈ0?«—M•ÞCÛ?8±³}?«—M•ÞCÛ?˜:î‰"7"?ˆwïQ'U?ï>(‹©/Ó?ˆwïQ'U?J̏j_¨?B='ÎÉÿ?ïùx½8ì?B='ÎÉÿPSR4FGL J0803.2-2522?±Í"Ç…Œ³@ùݧ¤À:ãhšô­À<0ãs\@…_ KúÕ@ª¬Ùè>B?Æ2šÜ垫¿' ƒ~áB·?Ð0¥Nفç@b"¼î]k?îR¼›&b¿åîs°Ñă¿êM=Ëg¿Û!L€â¯¿Ö—†"iÓ¿à"ÈŸ@¢‡UNASNone?ïút³¹³ô?@a±º×Ù?F-0-WÎf?@a±º×Ù?ïߨÇ&ß?"€e×O{¡?p+·'mÐd?"€e×O{¡?ïîRŽBM'?^+ƒ4R?a­q©Õ³?^+ƒ4R?ïùW«sÇß?0ø£¤™"?J¡RÏ4éU?0ø£¤™"?ïêÇ]~5?fZÕÓJ"!?e8£
s?fZÕÓJ"!?î×'üô1ì?¯Ô'‰Õô?¢€.),K?¯Ô'‰Õô?ïÓü¹Eþ´?~–ï+*ªë?v£Hbýù?~–ï+*ªë?ïÏí¸¢à?j@V)­?x	#'ØQ?j@V)­AGN4FGL J0805.3-7425¿×í¢ðÁõÀ5QŸ<pɗÀ;8rǝ¸ãÀ<‡TÂÏóÉ@x4`YÜë?ÿO²ZZ¿i?ӊÙÂÿn‹?Ôb'ÁÙ'?üµ]åŽd²@T"Uð¢¿ïû¨b4R˜?ï$‡nÊ?­âcAën¿äO
?¸¿ãÏJ ¸æ¿ïú;e0ÜAUNASNone?ï÷•"ß×?HWíJâ?PÕþö|àÝ?HWíJâ?ïëÁh¯Z»?gn{¤ä@?d>—/©]?gn{¤ä@?ï£{B¤,?~ú3<àŠ?‡!/v,ð?~ú3<àŠ?ïÑ#«V?\_Ý•S?wpýp:?\_Ý•S?ïò}VJ˜?Tá{Ë÷f‰?[S
Z'à?Tá{Ë÷f‰?ï¶iÉû¿²?Ž;µ¥ë?'e{³"?Ž;µ¥ë?ïQ~²YüB?Œ*7,?•Ð)­á?Å?Œ*7,?ï0"Ä9D3?‡ æCZ6œ?™ïgw«ž?‡ æCZ6œAGN4FGL J0806.8+5659¿ìÇ(B´'@@O+ý´Ì%À;¬sè/(âÀ<ôe;Ãûm@ Ó{d¥F ?û¯W™?Ön5Ó £ä?ÅöRT"Ö?ñWE+ƒ;‰@ï¾Î²U¿ïÿêf:Ç|?ïÿx†#›¿çöˆ‡ù^%¿»ñöýÍË¥¿ïÿ‰î*ëf?ïüÓZ…‡"UNASNone?ïö'[ {å?RM}QÅ?RÝI8W†6?RM}QÅ?ïò¦]¨R?Zíª&RyÈ?Z³úÃ~
-?Zíª&RyÈ?ïVXâÍÈ©?ŽŸÖa°{?•4㤏ç?ŽŸÖa°{?ïîåCJü?O/|V¼¿?a¼Ö÷ÔQ?O/|V¼¿?ïó)Ñ=Ry?Y׎) x¶?Y¬]§Ý¢?Y׎) x¶?ïÂòuþ´Ñ?€©ldž
{?~†ÅsË>?€©ldž
{?ïKª"a?'•˜þËè?–œ
­Æå?'•˜þËè?ï¤|…¦am?€LzùŽ«c?†àވ©4×?€LzùŽ«cAGN4FGL J0807.2+3312?ïY;R@=q
{é…jÀ;{ë^ˆK"À<Òâ'0ïŒ@{;B `ô@¡E= ó?Òå–È.›?Ò¢
a,ë›?þ$Ü=ƒN?ù<p>–©?ïþ âx°–?ïí5€†£¿Ë¤è'4ù¿æaµ&½Ú¿à_•'Í~¿ïû…LXžUNASNone?ïèŽPgˆ?gVÄúô½?gqøÚ3 ?gVÄúô½?îÊœl²±?§BÈ¡ç?£_Æ:»ó?§BÈ¡ç?ïtG­"¡ˆ?†%a)äŠ?'w
Tk÷?†%a)äŠ?î(ÎCEê?'ÒÁ9ï?­s\j?'ÒÁ9ï?ïÞ5Lèæß?p]–Ŗ}?påYsL¾?p]–Ŗ}?éÎÌy?Ë,äm0Á?˛¯ÀÄÎ?Ë,äm0Á?ÁëOø?›$²çÉRo?§–SÝÛd?›$²çÉRo?ç2Wj—oë?¶ˆŽê?ћQ*Ñ *?¶ˆŽêAGN4FGL J0808.3-5121¿äQÿ^ùÅÀ#ñÆónøÀ:p1ÆK©LÀ;ܽ:ˆ'
@h`©
*
@
	Ö¶[?Çî•ßе?¹–UGì?ó~5Å´ª—@G+ÇYx¿ïZ쐰½?ïݍyЦv¿å©mƒÐ¿è×_Y¬Å¿áWÊÂ0'˜¿á2€óUNASNone?ïû¢·
ÔÖ?8¾)¢¨\×?Au#V;ü?8¾)¢¨\×?ïÚo¥ÝÓ8?€e2l‹Yë?rÈ,ð$/?€e2l‹Yë?ïÀO`?|tHªPd‰?Øx;¢ÛÉ?|tHªPd‰?ïÐZÉ$Kº?`WIŒÁ¼õ?wқfúë+?`WIŒÁ¼õ?ïâҝÜ?gi\w;¬?m-å&ob?gi\w;¬?ï)Éýåt?±UF"2(Q?žšÆòíŠ?±UF"2(Q?ï(±®¨
j?"C«À&û?šéÊ.mîÉ?"C«À&û?íò7Ús? ú³ü°æ?°oA,h? ú³ü°æAGN4FGL J0809.8+0507¿ê‹µÞHË @3Áõ8%á;À:ˆ$?ziSÀ<@w¯<™@iIºß™@…N{ŽØ?х¨á`,»?ëtm$ƈæ@× eeµ@	ÒG6u\ù?ïþš¥2T¿ãœ \–ÙÌ¿ìÞî7€ ¿ë7ë(Øf^¿ïúžâXÐ&¿äC<àÛødUNASNone?ëˆ
=¢š?͜C
Ib¨?ÁßûË	u—?͜C
Ib¨?鑄' ~{?ÄÏqî"?ɹí·~?ÄÏqî"?ëtÕ¢^d9?§´|2¦Q€?Â,©v†o?§´|2¦Q€?êÍ׆0¨Œ?¥ÊŠ¬…žT?ÄÈ¡ç=]Ñ?¥ÊŠ¬…žT?ëp¢ÑÜ?Ã-ƒ'˜W?Â=t»Ïà?Ã-ƒ'˜W?Í?ÀÆjnD?ÍÅ3{W3?è°Îedo?ÍÅ3{W3?çß,ªû8<?³85­Í2l?ÐA¦ª	‡?³85­Í2l?Ȳ%K'?°à#¶{m-?éÓxö¿m?°à#¶{m-MIXED4FGL J0810.0-0505?êuMÆ@-Ùh">À;EìSzÑWÀ<˜(=5ët@h
0ëp?úÉoŠÑ€?édÝÀ$5?á¢ÛA"¯¨?ù·$#Ë·#@N²OÈë¿ïüœ¾g.b?ïåèâ­â¿ãÊh8Î}§¿ØߕÜö–¿è$½"Zm4¿ïý'!« €UNASNone?ïùyÒBÇ?D]f¼¡éÖ?KŠÁ	ÔÇ?D]f¼¡éÖ?ïÃ'¢â?†@qJ +<?~tl½È?†@qJ +<?ï"Aƒ¶‹ö?€qÖ'-²;?ŠïŸ}Êw?€qÖ'-²;?ïîîÆØÓ?pkÁü°†m?‹ÄD_w×?pkÁü°†m?ïëÒXÚ?fÈICaœÝ?då-ãm7?fÈICaœÝ?îÇÕJ?±¿²Qß6U?£ŽÒ´Jþ_?±¿²Qß6U?ï:ُuJÒ?"ZA¾1±?˜¤Îž×½?"ZA¾1±?î.;üý¹v?™@NtŽ9˜?­@/HŸ?™@NtŽ9˜AGN4FGL J0811.0-5636?çÝù<cÖÀ(´Jb#á‡À:&Š®DÀ<öÉ™"@i¥ˆ€@«"}¨¢K?Õr4ÐÂ$Ó?Â'}mi?ôò†š¹T?þ{ZÚ6x?ïû":ŒÃÈ¿çÑ;&F»¦¿çM<>ɚ¿ÖôF£ÓYY¿ïÿJ˜ª†Q¿éyéÐé'ÿUNASNone?ïóËZ˗\?QŸGÄ¿Öþ?XiJÔ"?QŸGÄ¿Öþ?ïφîq7P?€ÜrY¶E?x<ˆÖ' ?€ÜrY¶E?祈_1qp?lR[½ü?…œh04?lR[½ü?ï­ôÒFÖ¡?eEÄ¡'`¶?"'ËjÚ»ä?eEÄ¡'`¶?ïâ‹LÇ%e?j*zÿÜãÖ?mt³[6²o?j*zÿÜãÖ?ïY"`ʛ?ŸÄ›°2'é?"ÍsëÔÏ?ŸÄ›°2'é?îّÌú!Í?™Òç"Ùƒm?¢fã/ü.?™Òç"Ùƒm?í¹TEÐ?˜²ù«ÁÔ?²5[‡Yü?˜²ù«ÁÔAGN4FGL J0813.1-5049¿ãù	Ž¤À"">À:W^!ôFŽÀ;¿jК¸@}ã ÷€@ü*EMçê?ɂâˆuÚÎ?ÃùGÿóë ?ùlsßË­@·Uê™?ï_‰ÓRù¿çt¸Œ£è¿æŠP†*Q¿ì	ÜW"KT¿Õ©ºy
2¿ïý3!jˆàUNASNone?ïóþ`Ë?Tø?|ϬÏ?Xû Yi?Tø?|ϬÏ?ïØ°OŠú?züû÷±I³?s§Ø;âτ?züû÷±I³?ï£ÝT#?Eÿ‡?ë?‡˜µ+?Eÿ‡?ë?ïÔ¡}`?\¿]ýÑòe?uð/V"*?\¿]ýÑòe?mõ¸?6¸íªw?ŒØ¤{²Ä\?6¸íªw?ï1©Ë¿å?¤36¤†ül?™Êߟ¨Ëg?¤36¤†ül?íO}q¥y?¦í}™ÏB ?µ"F*¢9?¦í}™ÏB ?íÒ+‹@‡Ò?¡éV'KjÚ?±n£¦i´ð?¡éV'KjÚAGN4FGL J0815.5+6554?æÂ0wÓ@@'Ò^ÝÀ;Ýh1AÁkÀ=ûG3›8@!´u»îÙ?úÌ 4Ríä?Ñw~ý.?»À'׳…©?èÝAÄÆn@†újê°?ìDS­úпíđʘ?'¿È"ãw3=¿à·íu?¿ÄÓàR:µ¿Ü+Uc‰½.UNASNone?ïÿ†¥Ô™?´^"Œ o?%'¸'"?´^"Œ o?ïöDhËז?Ul@9?Sw.ÅÆ4a?Ul@9?ïñUÛm"?p ñPàyD?]ËTzŸ91?p ñPàyD?ïýž^'ö?"!¡ö$
¨?7Ðßé?"!¡ö$
¨?ïÿ,J?³$üG?~¢´¾.?³$üG?ïÕj¿Ÿ?xôwp'Ô›?urË^T?xôwp'Ô›?ïörñlÇÝ?j´Ìæy!y?S9®â?j´Ìæy!y?ïö´øÎ;?Gè?ÈÑ»x?R–"×m?Gè?ÈÑ»xAGN4FGL J0817.7-5258c¿ÑY+'LmÀ#:1…ýÀ:[6ÖUâ‹À;×ê¾O@8°.†{/@CºkáÐ?Úß©HcF ?ç/Xb—¤Í@Õ¸~a.ï@=Õø¬¤¿Õ#lì'dò¿Îv~6'·x¿ë–îÄnYz¿ê{åßBp=¿ïùV}»¿ãs_ÍSÛUNASNone?íßÊÖR‡Œ?¹‡5Ðoº:?±©MkÝ?¹‡5Ðoº:?í5ó"]3H?µ¢nÆB€>?¶Pfë̋A?µ¢nÆB€>?ìzÇ¥gâ?¦øW¶'|.?¼)NJÔÀó?¦øW¶'|.?í%D4YÆ<?˜8ñ˜€
?¶ÕÞ\Uç?˜8ñ˜€
?é6h8gi`?ͯ\ÏcÕè?Ë&_bZ'?ͯ\ÏcÕè?Üzäãy?Ó7ì¼	?ፎsuÃ?Ó7ì¼	?äw^ç~v?¼Y'£ïïù?×BÄ1?¼Y'£ïïù?Ðãánøä¶?¶œü?¸?çŽHƒ¥?¶œü?¸!MIXED4FGL J0821.5-1436¿Þ.µybÜ2@(×bùÊ[ÙÀ;\>GckàÀ<ï/a›M@C×Æ%ß@*,©¬6T?ÔõD䋅?íâ_ !¸@Jùe²€?û@»×‡ÿ?ïà/€ KÐ?Ú,¢'¼†¿Ý¯»/¿ïáB‡N=?êŒäIÁ2¿ïôþ¯çÝUNASNone?î'Iªèì?´»°TM?­‹e_'q=?´»°TM?èã©êczh?·φOZ?ÌqXVrb?·φOZ?ê5
Ü°x6?¯"úDÃî?Ç+ԍ>(?¯"úDÃî?ï·^Ñq¢?—üîj»¼'?Ÿ	'‰™¸?—üîj»¼'?çù	M¨÷¨?ËÒê9*A?Ð
íd®°?ËÒê9*A?ÇÎçæûïr?Ð æ³"?êFA$?Ð æ³"?ݶ"'œõð?ÂZ.u¬?á$µ·1…?ÂZ.u¬?äØrƒ'V?Ï{Úó<^f?×òOøÝU?Ï{Úó<^fMIXED4FGL J0822.8-4207¿ámR_.ŸâÀ±ÕQ֌À:4®'xbèÀ;twlH(@!fø1ªr@ÆcÉÓô?Ç^«œ{vC¿ VQ›S-$?֜TŸi'@@X·ˆB[¿îø–^ü³?îqBÝöð¿Ýû
'ç¿¿çô¯¼пЈÊÿÃE¿Ø«úú݁PUNASNone3FGL J0823.3-4205c?ïþSê°.ÿ?*†þ"Ž'?*ÁT"ÔÐ?*†þ"Ž'?ïîgÓ4+<?oækPÄ0?a˜,ëq+Õ?oækPÄ0?ï¼_бD?ƒõ  /ö?€èÑ÷,g?ƒõ  /ö?ïý¢æŽ.?)RìÕäu ?7âæړá[?)RìÕäu ?ïú=Ae6L?E_þìãá×?G
ú>Ÿ&?E_þìãá×?ï£ù'H_?¢¡ô1Êè?€È¯Š0?¢¡ô1Êè?ïdïeJ?˜Ùž3µ£¶?œ3b~?˜Ùž3µ£¶?ïî\'?"q?\~
s«±:?a£}µmÎ¥?\~
s«±:AGN4FGL J0824.1-6004?~2áì©À)wùÖñýÀ;W†Ç.þÀ<ªZÉz1õ@!ÄÀ:Çý@üÑ\~†?Ü
ËD·j?ïÿ±eh@.Ý}ôøe@Jöô=ª¿á¼œ2Ñ
¤?åRqâpx
?·sëÇkd?îÙ²X­@@¿èù"»¼Q¿æ‡Œ+ÕqUNASNone?B±Û?¢½nþG?Ðï""]$?¢½nþG?ï€Ë(Õ-¼?¤E®œe?Í5Õe?¤E®œe?îO_*KÇÃ?ž+.¤O¢w?«

]×8Æ?ž+.¤O¢w?îhö;[á?˜Ý79c_1?©pœN™"æ?˜Ý79c_1?îaJü0E?°r9¢Eâ#?®YëM©F¯?°r9¢Eâ#?ïCΗ–ú?®4†C¡K‡?—)"Ì?®4†C¡K‡?íO·Ðç8´?¥¾íÚò&?µ'Aw|_ã?¥¾íÚò&?éŽéðÓ?Á×F¥xA}?˃…ÄX<¶?Á×F¥xA}AGN4FGL J0825.6-5216c¿Èä9RNÀ oŽ\NµpÀ9¿MÈ	ïmÀ;Š
öÔT@/A:2@'âƒw?Êy@ˆ±>ý?Ó¶h\_ÒN@Ç>Ê€Â?ö#õ¶6ˆ?à*ڟg¿ß]e¡DˆÆ¿ê¾'¢O¥¿ï'Iž¯ƒ?«ØSœ<ê ¿ï•Û¿-ý¿UNASNone?ïÊ%'—?oæá®­¾?zít'f@½?oæá®­¾?í€Wn¯hÁ?»vC ?³ýD‰¨Òö?»vC ?í´~Ҙé›?žùÒô—»?²\	i€å'?žùÒô—»?ïTcÃÉ?…ý¾B•þ?•|ӌÅÐÎ?…ý¾B•þ?ï<æhÿ?¨v5¬Ù>*?Ÿxc8ëv4?¨v5¬Ù>*?×}Û]3a×?ÒFlƒêci?äAQfO?ÒFlƒêci?ç>âO?³³õ¿¤	#?уÎ;aÕÞ?³³õ¿¤	#?ã¤ì–Á£?È׎¶?Ø·Ú&Ò|º?È׎¶$MIXED4FGL J0826.0-0157?ï§'§
öc@3öˆœTÀ:­`#VF^À<u°ç"øp@ÜÞ'h#Ö@DÙMä?Åßïÿ¬Èö?³íDfŒQ?í./ˆƒÇ @ª6+‡m?ïýI1¢9¿ç>¨Fۆ¤¿áüHKá¿æøÒpXƒ¿ãÆôµ¿ïÿÓ?,» UNASNone3FGL J0825.4-0213?ïýá(	ō?%tSÞè–?0öÁÏâÃn?%tSÞè–?ïñìŽß?]TÇ©LÂ?\&â,~?]TÇ©LÂ?ïíºÑ€Ce?`ò¦ad?bE.F+n?`ò¦ad?ïôL¹Êš?;;.Ê`›/?Wýf¢hK¡?;;.Ê`›/?ïýÎÍá}g?,^;§³?1‰'Þ?,^;§³?ïŤ.?zâ?ƒQÙV™à?}-èíQ#?ƒQÙV™à?ïázs¹‹'?qöÿH˱?n…ŒI4‰m?qöÿH˱?ïÊõÄè§Ê?d®•	§(?z…}í«:?d®•	§(AGN4FGL J0826.1-5053¿îÔ6}jÀŠòQÁ"´À9ÝË£!hÀ;©Ââæ@ž3×Ú@I6'sg?Ä!Z˜§×?АA–£E@
Ä.bT@kK
¶!¿äïv_Ø­¬¿æðÉ+WœŸ¿Þïeþâs¨¿âŒèæÞÆÊ¿ïÿž ßt¿è««Ÿ«yUNASNone3FGL J0826.3-5056?íáõ2>
#?­'!NO†?°ðVm3¯ç?­'!NO†?ï>>ڎà?˜¡ù›%d?˜-ø?˜¡ù›%d?ìÇDžPÉ­?£ûŠƒޏ?¹ÅÛ
y²–?£ûŠƒޏ?îèŸ/t{—?€äûJÄ3s?¡v

Ɏ?€äûJÄ3s?âG5ÙV?É?&ÜbÂ?Ûq•ÉÖMT?É?&ÜbÂ?é(DµÅ&ï?Ê/¾&ÊLÈ?Ë^í(ëdE?Ê/¾&ÊLÈ?߶@®ÆÒb?»FHh|É?à$ߨœ–Ï?»FHh|É?æë½4B@±?´6âPä"?Ò(…—{~ž?´6âPä"MIXED4FGL J0827.0-4111c¿Ð0îáZ߆¿úköÉ™"À:"'‡V ÷À;‰Õ¤â¢ø@!«t0Ô^<@dïmâ?Î`R»Ž¶è¿ŠÄ©Šô¯?°:³ží/]@+áìõ?ã@JÞJ£'¿ÛçÚDY¡1¿é°Úþ¾·¿áírÊ!÷¢¿ÂN9žÝ%`¿ß¨bÑÜVUNASNone?ïù1‹­«?t¡'>Ó3?K9ÑYª?t¡'>Ó3?ïêø@ïø?qÊF»c¥?eÀ0	Ç¥?qÊF»c¥?ïÃDفn³?³¯Œ£{–?~]"WUêR?³¯Œ£{–?ïûl)ì/?2ëÿe¿P•?CžN¹n!?2ëÿe¿P•?ïçE…pB?q†âô¿À?h€º¼ˆ=È?q†âô¿À?ïh©!L	?£ë©$Èë?'êÛÓbî?£ë©$Èë?ï,N`íÌ?–øRç¢t?šv4É°y?–øRç¢t?ïҚ–i?r‰L³Ïˆ?v²¸B‰äÜ?r‰L³Ïˆ AGN4FGL J0827.6-0059?å~—eóS@4Å2¤—ú]À;lWÛÀ<™ã½ª@ 
ããê¡?üe2.?ÓÓMÅZ½'?Éۥá|?õªŽI@Öې	"?ïýÐ_ÿD¿ß:Ç|*óÊ¿æAIvk—(?¯Kì_ÁW¿çIéXÎG¿èsHÎ÷ŸUNASNone?ïþSÎÅ[¥?"Y\3"ê?*ÃÖÿU?"Y\3"ê?ïò=:%ÉF?]-~\_#?[…Œ"`ó£?]-~\_#?ïá!êØÉ?n7?Õ¦?nüÝÕîg‡?n7?Õ¦?ïö_C÷Ž?67›Îô ?SAw蛔®?67›Îô ?ïÿšƒ]?AôùImy?Œ¶›µ•è?AôùImy?ïÉ*gøU?€þåÕݙ°?{j̲4?€þåÕݙ°?ïÍÅV/H?~ÓEËø¤?yvIéœ&?~ÓEËø¤?ïã°1>D?ZÇ@(¬ß?lOÎÉúþð?ZÇ@(¬ßAGN4FGL J0828.4-4444?Âù^6}PÊÀ ¸Ý+¿¡À:|ÀØ£À;Ï™¹z
@ ÔÊCX@é@&?Ïø‰ÿr¼`?ë:I½cMW@:ð
­@]"N+1¿è¦î·`-¿íù䒼/Ç? ¼«³¿Ý±cºº|¿í½tŸå
5¿ïÿþÞ÷UNASNone?ÖlÇLüp?ÊjJ
a´È?äɜYùÈ?ÊjJ
a´È?âA`,?ÏÌðqu@Ò?Û}ÃçÃ?¨?ÏÌðqu@Ò?ߝó׎r?³d¡:͵?à1x8Ç?³d¡:͵?à†•§,æN?µË͝Š?ÞòÔ±¦3d?µË͝Š?»P}q¿?Áe–¶ÿõ³?ì•ð]±È ?Áe–¶ÿõ³?ÂÌ.ííó?ȱ†U7	?ëLÿ´D"ƒ?ȱ†U7	?ÆFŒ§ÿÊ?°3ßøÅñ?ên\Ö
}?°3ßøÅñ?³
óì#ê?£9ï²LeV?휡«¶Ó?£9ï²LeVMIXED4FGL J0829.3+3729¿ã¥ö!vÿ@A`mqóbcÀ:Œ»NŸ À<xÉÓI@§6õŠ†+@0ïVd£?Çá£Þìßè?ѐíBäE@Mjßqêÿ@ì؜¹´—?ëG™ò"í¿å¥Ì­ÃJ¿é¥ß™±¿îå7&ݺ[¿ïµ6þ™Îs¿àЏ¥UNASNone?ïåw7¼QL?iìæ•çõ?jˆÈ*ñ"3?iìæ•çõ?6
{?©¯ç_V:?¤vø	/Œ\?©¯ç_V:?ï½8–Z±?Ž¯Ùñ•]?œ(XôáÕ?Ž¯Ùñ•]?î
ûì°?'3Kޅõ?¯/°Q)ý?'3Kޅõ?ï[¸])%é?"IZ+?"ˆôaºzÓ?"IZ+?ãÔ0'U=Û?ÐÛ8º?ØWžÛU"J?ÐÛ8º?ëûü+gÀ?©I&ÔCþK?ÀàR`þ?©I&ÔCþK?á:²Æ'Ii?·'¢°dNn?݊šrÝm.?·'¢°dNnAGN4FGL J0832.2-4322c¿àáµó8À<œƒXåtÀ9˜4¦Ð¹ÁÀ:‡l¸K@ ½[8á@½·B÷ÌU?ÊV/wˆ¿g$b­@¸?¹í•W?@YBkàMÞ?ïü÷™Ã
¿èË÷º·!¿ê…ñxô¿å MÈ௿àùã»üšñ¿è!,À¨QBUNASNone3FGL J0832.8-4321?îûÃQÆ=´?±ZQ',)O? CÊçÀ½?±ZQ',)O?ïäÝ#Ôgî?w+zçÛ¦™?k"Ûú²'?w+zçÛ¦™?ê¬'ʹ?² t;Q•?ÅO`Õ¿"?² t;Q•?ïì,äd™?OdVÀ~u?cÓiì™x?OdVÀ~u?ï?«Ñv÷û?¦é*@g^?˜
…ÒØΏ?¦é*@g^?ïS»‹SR/?¦–ª†8Ú?•ˆŽ"Ýì%?¦–ª†8Ú?ìqя»[?­afî¾½?¿qs'%+?­afî¾½?ï,òͬ5?''"¤;?šoÁŸkAw?''"¤;$AGN4FGL J0833.3-4342c¿Ä¯áQ
¬À—)|Ñ÷À92\ça£‰À:T@ ¤		>@Móùa€N?âÝÄ6%Uû?Ôñ†U7	?ò&˜Ö%;#@í‹k®yÐ?íYÌúïõÇ¿éPCD"nÀ¿é$ó¿ÕÃk¿ß.^b6¿ëÏ*à~Zy¿æ‹¿m"¬UNASNone?è)øÕqê‡?Дt¬$`²?ÏXª8Uå?Дt¬$`²?ïæ¦þ›?sh"Ÿ¼?iYx£ôG?sh"Ÿ¼?å÷RW™L ?´t6›Ž	š?Ô[PÍf¿?´t6›Ž	š?ïÚðRA?\Çc}'Ò?r‡×mVõ?\Çc}'Ò?ìc<³Ã"?Â]ƒÖ[8W?¼æaç6í?Â]ƒÖ[8W?ïV<üEòd?§ Ïø3)Ž?•8`xù…?§ Ïø3)Ž?ç÷b¤²Hß?²yS­­öé?Ð:¶›nA?²yS­­öé?ï;ÌН?‰þfwr?˜¦bb?‰þfwr AGN4FGL J0834.9-4612?ìÞYHÌÀ¯"9櫛À9G6v¾À:¯"½i'@ &K¿ÆÿÙ@q̾Šë?Ëjß\qp?¬)œÜo,3?å¡ä¶Î^?þö-pülx?í4T€ŠÔۿ뮛‰]â3¿êj •6^¿á?&¼,k™¿ëPݾ¿¿â†œ1#Ž{UNASNone?èV´}ܵß?϶ì§ç?Î¥.(ƒ?϶ì§ç?ï^×£i†?¢5sŸ÷ç	?"%œ#3L?¢5sŸ÷ç	?åq]K«5?´µ`(œ?ÕDýh©•?´µ`(œ?îÿ(ª.'?ˆ‡pªÀ'? 
ɨ™Ö?ˆ‡pªÀ'?ç|Oˉ?ÌÛPôZ?ÑÕ`híÍ?ÌÛPôZ?ì,Í!·8?ɲÕæã
?¾™–÷JFB?ɲÕæã
?è€òIÅ,+?³³xû¯Ý?Íü6ØëOU?³³xû¯Ý?å]:"a²‰?½žÈ(^#?ÕEŠ×<šï?½žÈ(^#AGN4FGL J0836.0-5458?ÊÌÂ×¼¦À!	(¿;ê'À:SEùßTÀ;æÂW(@A&œÍ@ˆ!¢7?˘iñŽM?Áøü–'O?ô½áâއ	@Ûr±Î?ä•qì¬f%¿äègÝßÄ¡¿ë¢_:øú¿ã
+Í
dm¿èÕøÅy¿æ¤O QC¿UNASNone?ï÷'/Ò?NHRåå&}?PÝãnþ|$?NHRåå&}?ï؁j	j?}·Ðw5pl?s¿Jô"Ñ?}·Ðw5pl?ï§î—å??Ò_R/×?†8Ä}Ú­??Ò_R/×?ïÐΏ£)C?W¤z-Œj?w˜¸ý˜?W¤z-Œj?ï'UiF@?"ë/;…?j¾é?"ë/;…?ï:|Fç3ð?¦¯aïµå?˜°w!a´?¦¯aïµå?íŸo®àJ?¥¿n‡ ‡?³‡SÒØ-?¥¿n‡ ‡?íý%rU\ÿ?—¥ðȈ",?°ÔkJ
?—¥ðȈ",AGN4FGL J0836.6-6036?ïÒÓ:éÐÀ'õûmÊÀ;ĘÚÀ=Q΁ز´@ÙÁ®‹™&@'$·omv?Ùè—ä7Íw?ïÿºà¼ô@zœ™(Z'?ó¶Yh|O?ï¬;ݦ¹¾¿ÑÏ£@âH_¿Æº–ê<Ê6¿Ù£C;"¿ëØMú^Ö¿ïøg_µ0UNASNone?í^Jr¯Â?Áô8\Îô+?µ
¯B²³ð?Áô8\Îô+?à.q«FÒ?ÏC˜8Ï?ߣ©rÄ\?ÏC˜8Ï?ìÏ,?¥á7"NúQ?¿á‡ÞŸ÷Æ?¥á7"NúQ?ÒÿYPm£?°SÉM2Û?æ€SWÉs/?°SÉM2Û?ë=~é?N?Æú('Í?Ã
[†È?Æú('Í?Á¢î°?Äï9ÄFì?ë—|ÄSü?Äï9ÄFì?ç=ÌcgÐÁ?¶Ú}YYþó?фg90^~?¶Ú}YYþó?¢ã+"Ž(?'žyð_b·?îÑÍFç'm?'žyð_b·MIXED4FGL J0836.8-4638?ᓋOûôÀ»Ä?_'À9m.Y°À:°ËJì\@êv¹DÚ¥@<G䛬?É@tú¨Ó?²µÔ¶a{?硅‹Å›€@ÑQž?ïò÷ÙÀÑ¿í
°'z˜M¿åÆ ©T¿å³Æ)ñk¿æÁqN÷´Ø¿ïÿÊ»z"òUNASNone?ïì;(¹ÌY?qÂnÆM~þ?cÄ×íâ?qÂnÆM~þ?ïç{á*…?sw–™Ÿ?hí"L0RT?sw–™Ÿ?íåˆÖu:?¤Ög3΋)?°×ƒ¸Þb´?¤Ög3΋)?ïÝ×¼iþ!?Xì_ƒÛÁ?q!¸sÙ?Xì_ƒÛÁ?ïÌIäÇâ¥?€ÎcV?yÛ
­ì¥™?€ÎcV?ïf0•7ùÛ?¥(›m½ú?"9íSÙZ ?¥(›m½ú?íúB@c¯?¥'0(6¶é?°-ïüâŒ?¥'0(6¶é?ïDzJ"L?çRæÖ?ŸÇ	¯Ð>|?çRæÖAGN4FGL J0837.8-4048c¿ím@#ì'?ˀ.¤SAÀ9M1áú[À:µƒßóðþ@~;Å(@6¦Bˆ?Ç×Ñ7À‹¡?Æ$£ç"@߂±ö‡±?ë`s/¢"û?ïýAԋ³¿äè]_V¨¿çæ끘Æá¿ësP$¿ð?ïÄT=nöXUNASNone3FGL J0838.9-4056c?îXw/·R½?Â=С~Ñ}?ªxÓ1?Â=С~Ñ}?䫚·ô?Ύʓaœ'?֨ʐËà?Ύʓaœ'?éÚiøŽ"ù?®˜©?ȖXÅ°?®˜©?æÌ×Â|ÅV?³«Ï
U?ÒfP{uT?³«Ï
U?ì¾Ì‰äxn?Â	n#¡ß?º	›°Ü<"?Â	n#¡ß?²¦«Sj8?ÀŽ]8ÈÑô?í«*•wBy?ÀŽ]8ÈÑô?åTñ@kø?µàû820?ÕýV(?µàû820?´Z±¯î?¦ñµ·Ö?í|p©Ê?¦ñµ·Ö(MIXED4FGL J0838.4-3952¿Ýø¡ª'ÃÅ?ë»'ˆÛuÀ9yo/bÄÀ:Ó¥á¦x¥@˜é6ºÒ#@ÿ^Ö?ۺϟ:~?ãqbx›Q@jl»=¥@"©ë¡ND¿àq¶ùê¿Ü&n¿%oP¿ë²ÑCT§¿ìÕwácà¿ïûJ>³‡?ïë/=Û,âUNASNone?ê‹7Oå?ʔ'ÝÈ%Q?ÅӇ#þÀm?ʔ'ÝÈ%Q?ç¸Ýâ?Ê¡ûyÖÍ?ЎEÉÉô<?Ê¡ûyÖÍ?éO²"·?°0=@,‰Ú?ÊÃÅ5Ãu$?°0=@,‰Ú?뺟(Ï­?©*}RÍ=œ?Á¥ƒ\ÁL?©*}RÍ=œ?ä(Šk[÷*?ѱפ¨Q©?×®ë)H«?ѱפ¨Q©?¸¸¾!¡+?Äû'ñ^Ò?ìèè;¾0?Äû'ñ^Ò?Üá,fv'À?¶·š/zÅ?áiÌĶ ?¶·š/zÅ?½ÆUé…Y
?²£*/‹?ìG5BÏTß?²£*/‹MIXED4FGL J0838.5+4013?æ|÷ȁ—"@Bt# –x}À;žU9xÃÀ<Ò³‰.èK@"Ztâ*,#?ûA*ØÞ©?ÆʙÁ²'d¿—…ã{²Jb?Òr>¡ÑL?òh_ōh^¿ïÿÿ" 5•?ïÿnªØ†>¿«2Zp8ø¿åÍ}å¿ØÊE¾¦ƒ?ѳžþ]h'UNASNone?ïý`V¾
þ?7Ð²Ë`T?4ýK»EÑ`?7Ð²Ë`T?ïãsÆ›?wøDÚ+ƒ\?léŒݜþ?wøDÚ+ƒ\?ﷄ£é(Î?'7fœG3?'×´Œq?'7fœG3?ïÄfO¦l¢?i×Üôî?}ÌØ6h–õ?i×Üôî?ïù»'ÍzG?M²©Ó²Ó²?Iô¯³~²?M²©Ó²Ó²?ïkuЫm?¢=ÀÒYð?'œ1IZ.M?¢=ÀÒYð?ïµà5¤?"wßÏLÉ?'‡ò‰""À?"wßÏLÉ?î´åÿ	C?–oˆãŽ¼8?¤± ÝçÍ?–oˆãŽ¼8AGN4FGL J0838.8-4552c?ê­TƒÝ<(À©Ðé'ÿqÀ9]U÷ƒY¼À:2`Nq@ o]µ<ã5@—¿|'1ž?ß'kŸ
qÉ?ìÃ-±@`Æu(@qÕÛ>U¿Ôºªö¹/a?ê_ä¡Õ¨>¿êvåں̿ãá"ßþع¿èEÓI¿ïÿÙÔóüUNASNone?ۆaTâ?ÕÇñ5?â<ÿOUþ?ÕÇñ5?íYК¦y?Â=iÎP?·å1z¼Ø»?Â=iÎP?ã2S#_øÛ?³<wÌ⓫?ٛY¹@I?³<wÌ⓫?ê¥g˜<?¯¢db'ˆ?ÅjaŸÏ‹?¯¢db'ˆ?Îܹ‡~B?ÐO@ºìa?èzÈў p?ÐO@ºìa?çn\Žúã?Óýæwe3®?Ñ#GÌâ
;?Óýæwe3®?âÊ€xhû?µÓ=[–ƒÙ?ÚkÔÿ.
?µÓ=[–ƒÙ?ÓrmíæšK?Á#Ø!i² ?æFÉ	²Û?Á#Ø!i² 0MIXED4FGL J0838.9-2502¿íÀfÔd4¢@#¿¸jßÀ:ˆ[3,}7À<GĐ¾(Å@æ)ÊÔ¥@ºñ¾Ýa?ÒϏìTR?Ùz®ƒ?ýçdã¯ga?õL®Cõ£0?ïøbaô瞿àpLÎå«Á¿éí{˜ý'g¿è%LÀ¢ó¿ì'¬Óª7?ÖÅ|vs#äUNASNone?ï¬2—›¬]?†6n&Ƌ?"óZ""¯?†6n&Ƌ?êñÙLɝ?ÁÆ7îj¨?Ä8šÌÛ¡?ÁÆ7îj¨?î<`Œ5ó?—'éý	U"?¬9ÿèônÔ?—'éý	U"?ë¢l¯‰N?¤o8ßÿáJ?ñvMAÚÉ?¤o8ßÿáJ?îI"Y¹"Æ?¬µM¾Ê?«fÊfûh•?¬µM¾Ê?ÊV¹Èì¡?ÎhY®8Á?éjQÄ×¾?ÎhY®8Á?êW˜MY#?°`i4¡ó?Æ¡žË²›s?°`i4¡ó?ʈNᘐ?³'cïòt?é]ìG™û?³'cïòtMIXED4FGL J0839.1-4613c?ãÚ¾§ðõKÀ>‰¨‹À9q ٔ[lÀ:ªi³øÀq@ ¤ù9@FE^¯?Í'ØŠE>?ËHoÛZ.J?öñ§ãxu?ùSj…ÚÊç¿îcϝ·‹r¿ì "@º?î፞¹"¿æäW}•W¿æãyÌz¿êøsCÄ{UNASNone3FGL J0838.1-4615?ï$Þ\?§Ô‡QP–?Ÿ<< ‹ž?§Ô‡QP–?îóOu‰?­ÿH?ÌÙ? Ë©&<p?­ÿH?ÌÙ?ê9ýÀhC?±'J#ö»?Çþ^ó´?±'J#ö»?í==Úyø?£'a´Œ?¶ïnÀ?£'a´Œ?ì—I"?»¹€C *?¿ÏëG-³d?»¹€C *?묢/üƒ?Éþx…;­?ÁMuû@
ó?Éþx…;­?æëkR·?¶M_^TØ?Ò))ßÍZ'?¶M_^TØ?âÚV‹½°?Ä33?Ñ?ÚKSü脟?Ä33?Ñ$AGN4FGL J0840.3-4544?éÒ¹Ë4¾›Àp²˜À:±èkŽÄTÀ;ºB<»r1@#'½@è¨u?ý(&¶Â?É£{æÖ¿—çÁ<BGð?Ñ3¢÷¼:@ŠF~¾w¿Û¢<€cé¿ïùÔØ4	?ïgÖs>»ý¿àÔ&~ïʿ嘑AƒÍ¿¥µna\'PUNASNone?ïý-°èã?B ôÁ	1K?6—JíEA%?B ôÁ	1K?ïéÖ<&Î?r'HH?f)ᖚa?r'HH?ïÔ¶ ôþU?{©dzÄew?u¤ï†0ÁI?{©dzÄew?ïå\Ú1Ëe?a«ž=;?j£%ìq*?a«ž=;?ïùÿՅ$?Fk_ø‡N?HªÊ¡/·?Fk_ø‡N?ïsr`o¬`?£g娢a?''³óÂAõ?£g娢a?ïv§ËØà?'´@¹Ù€?'+¡¬N?'´@¹Ù€?ï§ù¿Û2ý?'H"Ôg­-?†äµ?'H"Ôg­-AGN4FGL J0840.6-3130¿×›Ø)_å@3Ð9h×ZÀ;Ué'9YÀ<ׁ›v¬@'1È$@ü.Êî¦?ÖÜAÿÿª?íøЁZ@ñ¯:ÎÄ@
$ùS¿ïþÊá:B?ïXÛch…?ݼ"C¿‹¿èÐMUhÇ¿ïÿôÕ÷?îb¿è¸¼UNASNone?ê.3*`?Â[†ùÙË8?Ç£G3VÐ?Â[†ùÙË8?èóy´ÖÈ?ȍ&â |??Ì2í,¤à?ȍ&â |??èùÍ÷?°r¼X\ù°?Ì»ûÌÈ#?°r¼X\ù°?èHO
ep?³%tÃFGT?ÏÞÞÃÖjA?³%tÃFGT?Önž:µö?Ì*Þ-¥Þ)?äÈ°â¥@?Ì*Þ-¥Þ)?Êh°e‰?͐ÿE‰»Å?é|eÓæ¾Þ?͐ÿE‰»Å?Òfºš×Bƒ?À	²Ñyø?æÌ¢²"^¿?À	²Ñyø?Íôú™ÊÓ	?¸DŽÝû^¶?è'ÁYK>?¸DŽÝû^¶MIXED4FGL J0844.1-4330?èr-dÅ°¿àíQÂjs;À9Zox]߯À:š‡–ü@Ãay@ y½[?Â?ÎàÀʊþ?ڂZbÌþÌ@
RÈ>Ȓ«?ûæ"KÑ吿ºÐûۃ¿ëéz'}¿ãÌôÀ0Ý¿í:­³N¡¿ïÿ~Ù#ó¿ïûR¼ev|UNASNone1FGL J0845.5-4327c?æüLeÍþë?Ì(l•bd?Òg4d*?Ì(l•bd?ÝÔR;¥âA?Í@	ЎM`?áÖâ-ß?Í@	ЎM`?å‡û«Þ?´ƒ¼s¦'?ÕÜðĨD?´ƒ¼s¦'?ä7¾Y†Gò?±TB­|/?אƒLóp?±TB­|/?ÖEÜíMÃ?É]iVtš ?äÝs‰Y?É]iVtš ?¨îè_ã0
?·s#?ù~×?îqzIß?·s#?ù~×?ÏàxÕmŸ?µvŽëeG?èáʤ˜??µvŽëeG?¨'µHӁ½?—ØÅ2âpò?îvÔ«œ4?—ØÅ2âpòMIXED4FGL J0844.2-4554c?×tö")¿ÿùyÔttÀ9N:¶~­À:³>Áï-@"#êÀӚ@
KáQ?ÏFªâ?уZ{w?ý«·ùÖñ?þQvg]?îyÞon¿å<5œ}z¿æe墆¨%¿çœ&;Ó륿åéÀ°3å¿ïÿî,˜å?UNASNone3FGL J0843.1-4546?ïI/^giq?Ÿcê•r‰?–Ú9ò	à?Ÿcê•r‰?î•r(͏Ñ?©h"{èþ?¦¨Ýuº·ä?©h"{èþ?ê¦ê#Ž"G?°iÅ©Ës?ÅdWqÅ®å?°iÅ©Ës?í¹³Ü՝E?''H™Kì?²2aå"[?''H™Kì?íA&¦æfÚ?²£ôNa†?µöÊÈÌÉ-?²£ôNa†?怄3D¿¼?ÐÎiÆ5¦?Òþ÷™v€‡?ÐÎiÆ5¦?å"'&,?µÐv˲?Ô×±³§óá?µÐv˲?ßãDfuf?¹ÑšÒSÊW?à]öLÅM?¹ÑšÒSÊW,MIXED4FGL J0844.9-4117¿æP¦•Dd"?ï l¡éÊ4À8ôÃóà7
À:ËeCP·¨@¤d[Ÿ8@±a£Êu?ÁSŒÄôç?Ò`…_@V=>Nð(@Qï x¯?ïÚ¨W¢~E¿Ú"uá-¬á¿éÃ}Ò霿èØRq¼Û¾¿ïÿÿ>¹ú?í쉖WZUNASNone?çwh3g'è?̝}7ýâ?Ñ/™0ú/?̝}7ýâ?ãŒãË
?Í<j&íÞ?Ùóîæ8iå?Í<j&íÞ?å«Q²õ¿?³÷îA²??Ô©]öšƒ?³÷îA²??èÇ󬊍?­×ÔÕ¿?Ìà1MÕËÏ?­×ÔÕ¿?ÞòµGR­€?Ó&Þÿ²Û¾?à†¥\V©@?Ó&Þÿ²Û¾?¨5ÉÐ	d?·¯.šÈO?î|£c5É)?·¯.šÈO?Íê|œCÿ?³Hɲ?è¿Å`Øï?³Hɲ?¶NÈ®è²È?¥)ۙäÛ?í6&ê>f‡?¥)ۙäÛMIXED4FGL J0846.6-4747¿ï?[…6áÀ½g\/«¿À:€vÙ{0ùÀ;¢&äpX@!	¬&9%@|Ą(ï
?Â"O5G_¿µÅ3{W3?ó²"ý[
@T€œGžÐ¿èei|Æ¿éƪß<;¿êúŽÜ§5d¿Ù}®A~6¿äCt~­0¿Ü.Ë$V žUNASNone?ïú'è0'©?M=mÚ΅?E¸_…19×?M=mÚ΅?ïá?µo'?vÊÛE_r?nÀJ¡yç?vÊÛE_r?ï­¿ª$à?…š¨D*?";æ¤Óù?…š¨D*?ïñ3™Š€!?KËÚ_|º?]˜ÌÕ=Ù?KËÚ_|º?ïÞH(t?uÏ4%Œ"›?püøÎÝB?uÏ4%Œ"›?îýò(s^?¬K8çÁßx?  Ýv6iÔ?¬K8çÁßx?îè$Èr†A?šªÊÐeŒ?¡}³{kPô?šªÊÐeŒ?ï$dMÝX‹?"·n=`¸Æ?›svDTîš?"·n=`¸ÆAGN4FGL J0847.1-5954?ïý‹x'¿À$••ÝLvÑÀ;cÉ
ûkFÀ< ë'+@!Ù0*Pš?ý«¤C@Çp?Ï-=û¹o?­Çƒêó:?âéóN@Ö?ÿ6±Ú~?»Ò6T/=¿íê͈ê?®%CÜMÉ7¿à¼{Eñ|¿æ¨ÊYUì?ÑÞÖO,þUNASNone?ïþÍZ"Ù?ߺ©Ö"Í?#/=®¥%Q?ߺ©Ö"Í?ïðŽSÑtŽ?`Ôà*™Nû?^ãWìcµ™?`Ôà*™Nû?ïôú›ð"†?EK='Â('?V
ÈØ4—?EK='Â('?ïî ×»é%?LÉ:KÖ?aß(ïÒã?LÉ:KÖ?ïÿüxó?Ég×É@h?`tÒ}?Ég×É@h?ïÄ«$JPö?'7xÄ*?}ªmÌi))?'7xÄ*?ïö`¥9éc?cËݚ—ž×?S>µÿ ˜?cËݚ—ž×?ïªHß©«?w³Pî\?…mÈOy??w³Pî\AGN4FGL J0848.2-4527?Òs&#'f¿ò´óý">6À9OðøûÿÀÀ:ÚßVø4@a±U¢ô·@C›0r?ÁM P+?» 'ÛŠ?Ò2ÚÞ2zÒ@ìIڔ‹"¿îƒ¿<ÁQo?ïéªS%A¿ç¿6ÁÞ[¿ãâ¾°ÕJ¿ê28A:
¿À\Þ'h#ÖUNASNone3FGL J0848.2-4524?ï°[€Àjû?'=0?Áj?ƒéƞOV?'=0?Áj?ïÓ{g íÙ?'$8¦à$?vBLo‰©?'$8¦à$?íI=ÄÓÔ?¦ȩ韛?µ¶ßÑa\?¦ȩ韛?ï¯;–Ñ`?p"][[4?" 1
}t,?p"][[4?ë*"65ú–?¾/ EtC?ÃU¯'(¦?¾/ EtC?îhuŠE¾¦?· ôë3q?©x§WX'¤?· ôë3q?êÉ
ìÖé?¯
$CÀÄã?ÄÛÔO€¤^?¯
$CÀÄã?íHσº?§ÃG´fÒÝ?µ¹ƒçþ÷?§ÃG´fÒÝAGN4FGL J0848.8-4328?ï]üûœL?Äñ€uÜ%/À8UëºÎ‡À:aŸ®†¨@ƒv‹w—ç@OÅÛAÖ?Áh™ Öd?Ã[#§¤õ@K#@¬	YBg?ïÃ>Ò£¦?â®
ŸOæó¿ê0dKÙó&¿ê†Âùå¿æ¦òèÀHZ¿âÌø6#
UNASNone2FGL J0848.7-4324?ç=èBŸ?ѯè¶kô?Ðá…/zÂ?ѯè¶kô?é±<æ?Ä&ï¥aEb?É;£g ?Ä&ï¥aEb?ão=¤jì?¹€â¨t?Ù!"·+È'?¹€â¨t?èöö‹%ý/?­\Û8?Ì$%ÓhF?­\Û8?ÖJòRÔtr?ÐÇ1ÑÎF?äچ֕ÅÇ?ÐÇ1ÑÎF?Ñs
ßø´Ã?Ðú[úŸ?çFy¥ž?Ðú[úŸ?ß)'t@Í?¼`óñåò?à|klEߙ?¼`óñåò?ÄИÚép?±"þ[Áðñ?êËÙÉE¿ä?±"þ[ÁðñMIXED4FGL J0849.0-2702?ëýt
•e@$óÛYXÀ:¡µÿ*íêÀ<*hþÇÜ@)=Úù@v»cýM?ÍZ÷¾=?Éë9ÊQ}?ú¡:wË@ÙùŒÉQ˜?ïûÜpêN¿ç©µ2&¿é/ýS}U–¿å7ÖeÒ°¿ïÿt¿Å}M?ÙÈÞÁ
XUNASNone?ïوÄìü?zâ#+?R2?s;û€¬Ê6?zâ#+?R2?ïÖWÂ/\?xªÓEŽŠ?tÔpª–ýÂ?xªÓEŽŠ?﯎Ïw]@?yß	ôþù?"L./Qø?yß	ôþù?ïՒÖSUµ?Yª±sÇÏ??u6"áSå?Yª±sÇÏ??ïe	ô9g?›$xìa"ì?"^Áj"Þ?›$xìa"ì?îƒ`i™™?® t¿šŠ?§ÉùgBUü?® t¿šŠ?íêqҚ?¤
áìÖ¶?°¬qjÁãç?¤
áìÖ¶?îJyCôݞ?•o{‡¬Ä?«Xk¿Ö??•o{‡¬ÄAGN4FGL J0849.2-4410c?íx'àÅ}"¿Ìl‡g½ÔaÀ9ŽËŠ­mŒÀ:ž¾®üØ-@Èíº@òâÆ3U˜?Ú®4Ã?©újꯋÉ?âÁ@Âgîý?ò²jž.~Ã?æ¤ðzPþö?ã²ç®6¿æ]Ç[sÄ¿ìÏÿ‡4<H¿¢Æ¾bHA¿ê\›A9†4UNASNone?Nk•G?Àⓑ€,?¦Çë²ö—?Àⓑ€,?î	Êqã?®¿ó­Xµ›?¦/c]Ð?®¿ó­Xµ›?éè²$;.æ?°Û2ãr?È]7oDg?°Û2ãr?ï7	°ƒ?‰%¹v…x?™üÉï£?‰%¹v…x?ëGˆ&‡O?Æs,þåÑ?ÂáßgâÃ?Æs,þåÑ?äç$ظ¤ˆ?ÒÊ´•so?Ö1¶NŽ¶ð?ÒÊ´•so?éÛICã&"?²g¥c?ȒÚðsgx?²g¥c?äâ§C±þ?ÅÔ]´Tõ•?Ö:±ãxœ?ÅÔ]´Tõ•8AGN4FGL J0849.5+2710¿ïé=nÿ½@B`'ݽµÙÀ;:I¥ÒÀ<š…&E'@Ɖˆ*@ þG™Å?Ñd}£Cç`?ÊÙ'#0?öS¡Qô¿@ˆ3û°'¿ïö
~C›?ï•Z0Fð¿èªq"'¿çq'úä¿ëK»%_5¿ïÒŽXUNASNone?ïù¡ž˜(x?G7Œx¼±Ï?Iy…O§1"?G7Œx¼±Ï?ï€¦?b<Z¨²Ü?`o¹+ÉG?b<Z¨²Ü?ï£ÐmHá?€ØéAøË?‡?‹ä­Ç­?€ØéAøË?ïå¬	]̺?Paé|ú]D?jSö£"'?Paé|ú]D?ïõ¤1x?Xâ#'æR?T·_|µY?Xâ#'æR?ﺡ¾N?ƒ‡í»lY?Wjî–?ƒ‡í»lY?îós+_™?•‹_(¶UÞ? ÈÍEºì?•‹_(¶UÞ?ïQš¢‹¹:?†Dêè,(ò?•Ì«±øtÁ?†Dêè,(òAGN4FGL J0850.8-4239?êï:@	? ¯ø×À8È.¤X9}À:OfµN+@ÿ¬)Ü@	}î$nt?Í(+Zå?è}´'l¤@«y"O¶?ù²¬Ñ~¿Øs©ÏqÿÙ'{#â³>¿í*¶W?ö¿ï¬¦Q8ø¿Ý©y¡Á¿ïçÑ­ÝUNASNone3FGL J0851.4-4244?çúñßß?ÒFí†Ô?Ñîö@A?ÒFí†Ô?ÁºT5rŽÏ?½³ ¶%bÝ?ë'jò£\L?½³ ¶%bÝ?ãQM™!4ê?³=}¯-T¢?Ù]dͽ–,?³=}¯-T¢?Èâ7;ù?´*ªë;ýÑ?éÇ|zò1?´*ªë;ýÑ?æ1Þô0'Ä?Ó©)ô?ӜBžúy?Ó©)ô?†óPŽ²?‰€¸Çé*?倫2ôÁU?‰€¸Çé*?áåzh?»Ýsk»¡?Ü5ÃÕÇ1?»Ýsk»¡?`¼áõäUM?g@
‹æÿÜ?ïïC/7r?g@
‹æÿÜMIXED4FGL J0853.1-4407?æ2<	4uí?ֆsa¡…¡À9pNŽÙL7À:ž¢¶xÍq@åÿjþ@Œf«/Ä?Ð%lZþ?áf¦ÈVE‡@ÑÓ¾X•Ã?ÿbÄî‡Å¿èØ?ò‰J¿³ÓÿÆõw¿æ%"CïC¿ì(¬A<
r¿ïÿ|¢gô[?îÜ'éSQUNASNone3FGL J0854.4-4404?ç`¯°\S¾?Ëÿ<¼?Ñ> ŸGX"?Ëÿ<¼?Ø^Ç'á?ÍÔâ/Š‡-?ãÐþœlv?ÍÔâ/Š‡-?åewó£ó‡?´6|eڎý?Õ5¸ò?´6|eڎý?åÉ/»¯n?¹

Ë;À?ÔmÅ ˆ¡$?¹

Ë;À?ÙWÏ?íÝ?ͨµ«Èñ ?ãT`t	?ͨµ«Èñ ?"çk¤?ž[+¡xÉ?ïc—ÈšIS?ž[+¡xÉ?ÄÒ`¨"ç·?­têzÂê?êËgÕÚÆ?­têzÂê? V˜DL9?—kÝ[«Æo?îúžÆmüÍ?—kÝ[«ÆoMIXED4FGL J0853.6-4306?ïä¦i¥yæ?ñ%ð¥)À9
OH<¯´À:'²jJ÷@RÎؕ­Ò@ʁ~áS?Éj )?åÂ:¢"=@I!ßyx?ôIYˆ²l?›ƒi+'«¿ÖO'Ÿ,*«¿èeàš	+"¿îÞ§ msK¿æ©n)©G¿ïù>/GìUNASNone?ЫYX?Ðép_A6µ?çª{ÓyÓð?Ðép_A6µ?¸ÿ)
Nùá?³ pÂB¬¹?ìàÞcß4?³ pÂB¬¹?á5û=è1Ç?³¯úÏ~¬?ݔ	"/œr?³¯úÏ~¬?µZ"û?¡5@¬Ä›?íT¿}?¡5@¬Ä›?àÀuæáöÖ?Ò"˜€•?Þ2<U?Ò"˜€•?"-&*î_~?†ª~zK¤?ï¯Kg\…'?†ª~zK¤?Ú²ª'>?¾3ü,œý8?⦪ðó·a?¾3ü,œý8?MtàÄAÌ?Knë<­vª?ïø¢Ç¦ÙY?Knë<­vªMIXED4FGL J0853.9-5501¿ï¨Å¨ZÀ!º^5?}À:¡îM¯À<
'Á8D@ºSç2Ԕ@þtYœT?Щ•$¿Òé?Ñ*¢ëÒÌ?üíV•8	@ƒt¿±?îûa3v¥¿áÖ!_K?¿äK›^ëÈ¿ç&#€7ÈĿ런9F¿ïöI"]ÍæUNASNone?ïÁ y»5~?|â
Á6?/Ãw"ù?|â
Á6?ï˜Í¿™'?'gaP6€?‰Ì›»?'gaP6€?ï×=‹s3?cî2v?ž%Eú"¸?cî2v?ïIvhçõó?r8A:·?–Ñ2ãAŸ?r8A:·?îµ³ ÖÏ°?žn^	;?¤¤Åò"?žn^	;?í¶¡Ó,•é?·cÑæ±F?²Jñe¿i»?·cÑæ±F?ê‰ "Ò.®?°®ìݦsN?ÅÛ}ì·EI?°®ìݦsN?ëâáO˜?¢³H¹¤ž?ÃètyŠÁ¡?¢³H¹¤žAGN4FGL J0854.8-4504¿Â.ù°¹#€¿¡MŸßȖÌÀ8"Š'¾ÙÅÀ;H"ÅõB7@üíåKHÔ@
™#R ?´7¬"ž=?Ý/0ÓÊ@#ƒn—?üL+ín­Þ?êñ"¢A]î¿Û£iüóÜ¿Ê÷Ÿnc‹¿ã´k!a#±¿í]¶>•çÞ¿ïÿ³^¼£àUNASNone3FGL J0854.8-4503?:
äÁA•?4µŒ°À©¤?ïü¾£OŒ?4µŒ°À©¤?¯A¯ål?§Û‡Y2ó´?îåj¯?§Û‡Y2ó´?•*˼ž¯Ã?»l¼½?ïV©¡ñÏ2?»l¼½?…ꀗ'"?s5Að®0?ï¨Uý– ò?s5Að®0?NúUŒhÃ?9ÍwŠíœ?ïø}Á2 ?9ÍwŠíœ?€ýWQ†?'GŸß(y?ï¼ÞÒÖ?'GŸß(y?…ÐÌËEW?uôî>`ˆ?屮̛ñÛ?uôî>`ˆ?&¢ÏâÀW?ls"-?ïþ•Òî,¡?ls"-PSR4FGL J0855.0+0720?â»tŸ±ƒ@>Åé\îÀ:Ã<«ùjÀ<\R±}»î@
´t:å@¹™Üµx?Èx/çyKp?‹Ì*IP?¾)lµàÍ
@ԆλºV¿Ìєݝ)œ¿è|u éY ¿ç[i³"¿çêï͂Õ2¿íÁ¶ÿ0![¿ïÿï9_JUNASNone?ï÷pdõ€©?I*BŽè?Q5ŽMÿF?I*BŽè?ïï3¢x÷?jÜxXW¸)?`Ìbœ¿Ø4?jÜxXW¸)?ï¶:††?uiÃîwÜv?~¤âÚIœà?uiÃîwÜv?ïëïrzW?MŖ*»ê?dðwˆ)?MŖ*»ê?ïøÏ1r?H›-è2ö?LÃ;Ü5z?H›-è2ö?ï¿ÐèãÑ?ŒT'&ÔBF?€ýí5¤?ŒT'&ÔBF?ï¼ù6¦ôæ?€—‡Ýö?€Á²ZºD?€—‡Ýö?ïb"QŽ"?²Éÿ¥{?"»µÊ¾û?²Éÿ¥{AGN4FGL J0855.0-6026?àa*•ˆp…À#µKjaªÀ:Ï,?#+~À<U™OǾp@Xš]¹Ä‡@ôº¼ÿÐ/?ÏGRúν¾?Ñ*ò‡qxé?ÿV­ÜF½T?ÿt'Ln¿èã'Á¹m?í£†ŒG!¿Ü~óûå¿¿âò(؇¿éÔÈ¿L½¿ïùé€aº/UNASNone?ïâL;u'?d&{qä±?m³Ä†`æw?d&{qä±?£òID?Œ‰­™Â?‡×
¼'Ý?Œ‰­™Â?ïhŽ"'Ùd?…àZ3­J‰?'î-v"€?…àZ3­J‰?ï>h{È?v½ ÝÏ4K?˜2ðß5·?v½ ÝÏ4K?ï^š[F«?"ºZŽÙ?",¿'Ž?"ºZŽÙ?îAªl*P?·¢££ô?«åY@Ñ?·¢££ô?ì¸2
‹–™?¥>æc¯yk?º>o«£K8?¥>æc¯yk?ë/Xy­"Í?©KÍRÁ‰q?ÃBžIìÍ?©KÍRÁ‰qAGN4FGL J0857.0-4353c?ޚxÈyè
?ð'Ú:s™UÀ95–4ŠKHÀ:}NÏpëû@¿ÃJB~@6&}BJþ?Ò#1=9ÇL?Õ¶¥ä*·d@۔XÖ[?üo|½?æö?ìåÁX¨8¿×"›¾7Ô¿æ"Mºö ¿íG¨€gC†¿æ4óý">6¿ïÿ
Çhß½UNASNone1FGL J0857.7-4345?åß^âZõç?Ó@Ώ£)C?ÔAB;J1?Ó@Ώ£)C?âL¿(th]?Ï9fÓô‰T?Ûf¯/G?Ï9fÓô‰T?ä[(Âz?µñÀ¸q"û?×I¯áÚ{?µñÀ¸q"û?äé'BÒë?³""SX¹ø?Ö,Û{øZ*?³""SX¹ø?âhWGÃÇ?Ѿ¬p-\?Û/QpyÔq?Ѿ¬p-\?¸<>¼V?ĉV)œ?ìþ˜xv"5?ĉV)œ?Ý©f¹¦?¹0æâ(§à?á+L£,üt?¹0æâ(§à?ªìò»e? ÉO¥ëÈ¢?îQ0ÔU¤š? ÉO¥ëÈ¢<MIXED4FGL J0857.7-4507¿ßpà¢â‡?Ôð°lCõùÀ9_É'%Þ·À:¯"¡@ÿi«kG@%³Æk‰¼?ÍÙB¼h%®?­N—½¡a?ýäJ|ûÔ!?þ`Z³«¿äý ¿¨¡õ?ï
}—"ã¿ëfx¿âyì?®ÁŸ¿î–#ùŒ|¿ïÃOÀ²0UNASNone?î±7å–êŠ?°L
Ð&?¤ì§m>]?°L
Ð&?ëk°'
Ô?ÁCÑ0^ƒ?ÂQ=÷Ô¯½?ÁCÑ0^ƒ?éðMoõ[a?°á¤Ç¶g¥?È>Ê@*'{?°á¤Ç¶g¥?ìi—Oß³§? û…¾`[?¼³EbË? û…¾`[?â¬W`Ü[-?Ð&DÂý–?Ú§Q>GI§?Ð&DÂý–?ÜüÊåÛ«Q?ÔIK¸E?ၚ*X?ÔIK¸E?ã°_þ17Ÿ?½*,›¶Ì¨?؟@Á?½*,›¶Ì¨?Ó5[íø§­?½×´‡[©t?æeR	¬)?½×´‡[©tMIXED4FGL J0859.2-4729¿ã×:@š¿ðn*¦€2À8ŒÓa;";À:'
—~6@&®¥Ô@Âä›ök,?¶À:Çý?ÅÍÛÕÿ%@
èþüÊÁZ@ße»Æ•?ìäÀ™+¶¿ÚŠžc˜V¿æŠâ¡ö4z¿çì2"'û@¿é"¤!²Ø/¿ëbZ¾ž
UNASNone3FGL J0859.3-4732?å_ƒèF>Â?Ï$á}LÌ?Õ@ø/s'{?Ï$á}LÌ?åKùÐæâÎ?ÈS½\ ?Õh^2:e?ÈS½\ ?ãÙw¥?¶d§'g?ØMµÀýÈ?¶d§'g?è'wï(?¦ñÿ×Ô!?Ïb#ìC_¦?¦ñÿ×Ô!?ÇÙ°‡a?ÄS.Nj?ê=ɓÿž(?ÄS.Nj?¾‹'\k?Åz£A/—•?ì?N½Ôs?Åz£A/—•?ÑNOòx®?¸ò)ûíoÜ?çXØ~†Ã©?¸ò)ûíoÜ?¾(ͶyÀ?£Ê&*Ç?ì:æI0ܨ?£Ê&*ÇMIXED4FGL J0859.3-4342?×-rKn`?÷]qËväÀ8¤ç2© xÀ:Š·y¥@‡BÈÒlI@쭀k`?»@|`½sØ?عïºãkJ@9#'Õ?ö‡ÌbCÁ÷?å°8!Y–õ¿ß|÷7¢L¿ç\ž ¼ã÷¿êWÕÿïýÄòã¸?Уi&4G/UNASNone?¥¨ûž\Ò?±müIÄ?î¥pF'ñO?±müIÄ?·'$ùźp?±»]é´ø?í»`''?±»]é´ø?Ñëó'CT­?·	Ô
›?ç
l^U©?·	Ô
›?°—ÝCø?–Ûk(˃Õ?íýlÍ]Á?–Ûk(˃Õ?'äNST?°à¶/C½Ú?ïhß"KÕ?°à¶/C½Ú?ƒ}ý:	[?… ÇcÀêw?ï²°.ÓÊ?… ÇcÀêw?±c͟烶?¥·-CQQ?íӆL,JÙ?¥·-CQQ?Aö
N´?4´÷ÜyÅ	?ïû˜¹í"?4´÷ÜyÅ	PSR4FGL J0859.8+0053¿Ï—¥»2gÿ@<®Ü]cˆfÀ;9!‰½"À<¸d(ž"»@"¢ªÜâïy?Ô*"}ÙI³?íEÝYâÊ?ïÿÕ7ÕYc@žÁÁÖυ@B)"â?ì»m߁…Q¿Ó–Ñþèk¿ïÿ4Þ®÷z?ïñ
žÏ
š?Ù·`9{¢¿ãÊ?wåUNASNone?íÕ®r;(B?ÈwýÁÑ

?±RŒop˜r?ÈwýÁÑ

?ïò}†©%?a¾ŒuuI?[󮲶C?a¾ŒuuI?îïð'£?–îæÙçˆ'?¡÷ñšŠÑ?–îæÙçˆ'?ïýc-?2"væûoø?4çþ€rÜä?2"væûoø?ïWD!åO?ž2ÿp]í
?•—v›ì?ž2ÿp]í
?ïÈò¢'Ý?ˆ»WÀ—p†?{†þ¸]y5?ˆ»WÀ—p†?ï…ñ_íë?•ÄëÓü?œOAÔB?•ÄëÓü?ïúxªiS3?TÌYcŒU?FUH_0Ä?TÌYcŒUAGN4FGL J0859.8-4530c¿ë®ÇÃoù/?Öù¾'BÀ9.Ž'uÏÀ:§†S€@O›æ¥ç@¸1ôo?ÔùAÀÖÌ?î¨Ä_@x@£ßm¹@ÿ?þN>&I¿Ê"ù#—ß°¿ÅuB⨬1¿ígß7]¿çڙz"¿×¼Zcα~¿ïûï¯OäUNASNone?çæM"ö¨?Îò›w"	Ô?Ðä3dö°?Îò›w"	Ô?á"_Cî}ˆ?β(ïëéP?ÜÙAx#ð?β(ïëéP?æª"W»H?³ê(3?Ò«»P‰Áq?³ê(3?ç´F™'?´ÕÄ,R3ù?Ñ̗rÍÒÜ?´ÕÄ,R3ù?ã¢Ái"P?ÐvÐÉӖ?غ}ñ-»`?ÐvÐÉӖ?©S»J5?¸#Ð3¸?îjÃÔfÛ=?¸#Ð3¸?áÜZì,0?µÜTç#j\?ÜGJ'§Ÿþ?µÜTç#j\?´:cZƒ´I?°Ÿ'ϵfR?íx³"†N'?°Ÿ'ϵfR1MIXED4FGL J0900.2-4608¿ïÿºÄÑDš¿†* Û[ À:Ž‹µ«HÀ<hõŒßw@a~#òM@'ª\_|g?Ò|Jž‰Ãc?æüÑA¦"}@	âšÛ¸ù?þUºêw,²¿èÌâÑñϼ¿å¿SÒå낿ӷè99Ýq¿åÇ¢'¿î2ÜÌQ¿ïÿ'Þt†UNASNone?çeÝs–®?Ç/;;P?Ñ5ÀEÒ¤?Ç/;;P?èM™+ñ±š?Åú"Šòóä?ÎɛP99™?Åú"Šòóä?ëpc¿0ñ©?§ß?XÒ?Â>q<9[?§ß?XÒ?çéV
M¶Â?­ø1 #0?Ð-Sëd'|?­ø1 #0?؅%9±½?ÍVˆ¾¼$?ã½mc'9!?ÍVˆ¾¼$?ɘ³."çu?Í[>™\¡°?é™Ó4^Æ#?Í[>™\¡°?á_»T)wô?ÀÈd¤*¨[?Ý@‰W­?ÀÈd¤*¨[?ÆDúl(ƒ?°†âCÒ5?ênÁdõß?°†âCÒ5
MIXED4FGL J0902.5-4727¿ÔJNd´W¿âŒ0êÄ/À9—áZùJÚÀ:Ëu$oK@ =¢wä"@U
`¬B?ÆíÂ;?…Õ£òQ5?ÄøŸ£ô¼U@ÅKSuÙ¿íék¾êáá?ïî5gÀÙz¿èQˆ˜`´¿é5#˜‹| ¿á§a8)<9¿ÛoÑ~ã4îUNASNone1FGL J0902.5-4731c?ïÏjö1äÃ?Š"f*ë?xJ"ö+æB?Š"f*ë?ïßÇNÄÅS?z.N|LÈ?pX½éªˆ?z.N|LÈ?íw^1tÓM?§
¼ä®]?´Ev3—?§
¼ä®]?ïæ,Žm/r?V¿W'\ïO?iÓqdÞ?V¿W'\ïO?ï)I_?šRTƒ|"?šßVÕ3T"?šRTƒ|"?îåßIôb4?°KêλEƒ?¡¢`¹Ü¹?°KêλEƒ?ì&lmçd(?¯öw_ðÆö?¾ÌœÄÞÂ?¯öw_ðÆö?î÷ /ËIÀ?–>Wmhýß? ý·¯?–>WmhýßAGN4FGL J0903.5+4057?ÑÂz_¼@DÚË}At?À;­RÜEæ"À=û¼¤`@ {åóìÌ?û¾Îø 7®?޼ɴêWø?ÆÂx¡[?íìw¢xæF@â!Üɚ¿ïÿ€H»Ê?ïõæ °Ï–¿ã¡Çe"¿¿Ø»;ÀJˆd¿Ñ5¡l犿ðUNASNone?ïýU²]¥?+Ĩú$D?5RmÍépª?+Ĩú$D?ïõ""³‰?Tâg
÷ú?UºÖñäíT?Tâg
÷ú?ïÙ{F•2?sú#öI?sBsïCJÕ?sú#öI?ïøŊÒñ?6È3."c"?LéÔ±{ð2?6È3."c"?ïü¥"|'?7dMï¿?:×ÃYèý­?7dMï¿?ïϐ	‰&ì?zåû"Oû°?x7ûQj	ð?zåû"Oû°?ïȒ^£	Á?(@yäeÏ?{¶Ð«»o?(@yäeÏ?ïâXÇQg?bž6÷Œã¯?m§8Ür¿?bž6÷Œã¯AGN4FGL J0904.6+5200¿î²°%]@D§<`ŸÀ;X*CbÀ<Â?Úác@?o¾Â@ÚCä'?ÊÇãÍ¿¡6rWá=r?Õ[¥BDH@
ûx¹ u?ïõõòðM¿éÑ(| ¿àœúAzÓ¿î›;ùç¿ïÐlÊ-¶?ïÎèӓUNASNone?ïþžt'wÇ?]*SÓI87?&½ôD M?]*SÓI87?ï÷iÉÐ̔?Q˜y[?Q,l'"Ç8?Q˜y[?ï´e:|C?3`¹V?'æ±oº%=?3`¹V?ïýxg…Ã?"EqMŠdÈ?4?"Z?"EqMŠdÈ?ïÿµË\?w'-w³? ‹3^?w'-w³?ïׂ9øìˆ?vµ5`ðr?t>ãwwÿ?vµ5`ðr?ïÃÎ*3Éö?'ÌË|ß?~êæÊñ?'ÌË|ß?ïñ‹žŒÑ?PË=QÙ_W?\èà Kó?PË=QÙ_WAGN4FGL J0906.1-1011?ëæåÛD@7ä=F²køÀ;ÙÙ$ÉäÀ<­¶‡*@üÎí¹Vx@Vçæ-Æã?ÇyåHn¯?¥³Ûd?D¹?àE†6`å?ñ¸'Æ@Á'?ïÿWߣ¿êw?&±p¿á"g¾U:Å¿âvYޘ§+¿æx²™Dà?™ü%]1šUNASNone?ïûHd}ó?>adÃ.¶O?BÞ•N?>adÃ.¶O?ï¿F߸aÜ?†7œÅ
E/?€.H'Ù?†7œÅ
E/?ïÞ#QÇP•?qá¬Y?¯?pîW·®?qá¬Y?¯?ï€6Z[m?q_d½b'F?òi~À³?q_d½b'F?ïùéÈÛük?J×PÜ:‰i?HXÝkõTR?J×PÜ:‰i?î­_jrv?®Ü\7¾|5?¥*)XØ£?®Ü\7¾|5?ïÙÿ=zã?w¿4>96Y?say¢±?w¿4>96Y?ì§ÈÆǔ?¡Šæw"–h?ºÇñ¹ÉÃa?¡Šæw"–hAGN4FGL J0906.2-5337¿ï÷o{kŽÍÀ"?Åè­À;ƒÉØ)øÀ<žæs.Ì@#XîßFL?ärÈ^þèÿ?ôP|V?ïõJšX{@["UU@ӌ1Q0Ê¿ïþÜêQB?ï˜Ê õîÚ¿ð?ïÿÿ&¦³?êbÙHÜä¿àC ´UNASNone?ï¥ÂÏÈ՜?³xÂ.?†L
ʘë?³xÂ.?ïèp€+?wvi-^«?gà¥	œY?wvi-^«?ïUmJ0OÔ?'µ&#;™?•RV´Î›‡?'µ&#;™?ïÿLy*cV?»M
YÇ?pڎ£´ ?»M
YÇ?ïêúƒÐk?o\á®avð?eèÍ=?o\á®avð?ï10aq´ù?¬þÓýev?™Ùóب˜Ó?¬þÓýev?ïJ§X]?"¸Kh£?–«º%U?"¸Kh£?ïü܀ã¯?FŠ±Ô¯/?9÷ _ҋ?FŠ±Ô¯/AGN4FGL J0906.8-2122¿èŸCYÆðÀ@1.¿üÚ±'À:'ŏÁªÀ<NÐ& û@F»Å™5@ÎC$Aþ¨?Ä°uh·Ïe?ﶰËåF@@Vý<×!?ýÐ$ˆu…¿Øå#»qп±áêìžF¿è×Obîœj™Ñ;¿é>"Õ½6W¿ïk|»<'UNASNone?Ä,Ð+Â`?ÈĆfOÙ÷?êôËõ?h?ÈĆfOÙ÷?Áȁ³Ì?¾•	sé~+?ëß"<Ìÿ?¾•	sé~+?â	ˆ&ՁÒ?¶ÑT³)%?Ûìï²Tü\?¶ÑT³)%?®D]ý1?•Bõ=ÇEU?îº !Þw?•Bõ=ÇEU?§Î*EÓè®?¶‰ºý! ?îƒ[°å?¶‰ºý! ?œ\=°Ÿ •? š*(Á–î?ï²»? š*(Á–î?Õ¸Ýô‰Ì"?¸y@ÐÙ
™?å#'»¶?¸y@ÐÙ
™?PsÌa2A?B½¢+ìi¯?ï÷Æ̧/?B½¢+ìi¯MIXED4FGL J0910.1-1816¿ÎöÿlB"›@3¿.Y¯ž¿À;)t"&"À<™™'óe@ U'}‹Q?ú€3çŽ3?Õ?¹=ùµ¹?áÒáïsÁ@¦"¦óõ@N·[÷M?îÖì
µÃ¿ïûÉeeà?ï³t'Ü¿¿Ý~ŽÑ¿{¿ïømÏç3€?ïk²ÖuUNASNone?ïõ'ÞÂ\?S¢'
æû-?TÝÉÄ	§Å?S¢'
æû-?ï×¾U:Äø?}.U"êŽ?t ÕC±5?}.U"êŽ?îò°œÉ?¬$]^? ÓÔòÃÓë?¬$]^?ïD͜Ödü?ˆ\uV+KV?—fLaÃĄ?ˆ\uV+KV?ïæ¡ç#™?mãÒbŽñš?ið^'ú¯,?mãÒbŽñš?ïq["ü&?œý\'ô?'ԍb3
å?œý\'ô?î*M_É,?Ÿ:·Ô³…?­[*¸F?Ÿ:·Ô³…?î¦Ã½sW?¥ŠðT(†?¯E"À¹.?¥ŠðT(†AGN4FGL J0910.9+6055¿ì}èU¿O6@D:Ü
²À;€Åt÷TÀ<îÈ8–@³Bâþ'?üiÇ)Ý;?Ô¥:´e?Õ¥óD/Ú¹?ÿîãª2n@·7œ¤eû?ïÿÿ^ðP`¿íõGàiaÃ?×de$œía¿ãí:`Nq¿àq9~%õ³¿ðUNASNone?ïù˜Oá?@/]ˆÔY?IÂÐùòë?@/]ˆÔY?ïñéµCvÖ?Y$3
Kaî?\,•¥
T?Y$3
Kaî?ï¦mL´Ž'?€ÛZߢý?†d¬Ëý#j?€ÛZߢý?ïȦï1ju?_q´¡ÕvÃ?{¬ˆW|'•?_q´¡ÕvÃ?ïû»pÀÄ?@_H¹/Ì?A=ÓHߑ?@_H¹/Ì?ïÈ¥Ë" 
?{ÈaJÎ%'?{­bQbÚ?{ÈaJÎ%'?Ib±?Š–²i4§?Œ–X·ö'Ä?Š–²i4§?ïd!)ñ@?'K4Á†¨:?"{ÚÀ .-?'K4Á†¨:AGN4FGL J0911.6-4738c?èH'`²j?ۀWÿ|ÙÀ9
!¯éÀ:ÅËÉdc@O9k²r@V½+o"?Ñ,B]ó{7?θ3b­õ?ú|°Švæç?úr¿¨X¤?ïïwâd¹"¿ÐØ
]5»#¿ìk–@ô'ã¿ç©&¿ÝP(¿é«Þ…_?Šú)"ç8'UNASNone?îãÀÒ+?ª‡	BJ²"?¡ÃÎöP?ª‡	BJ²"?ìùùo†å?½äü:ðä?¿à04ƒÈÕ?½äü:ðä?êeLóòß?®¡r ÄKÃ?ÆjÏà04"?®¡r ÄKÃ?ë÷¿ðyý?¡m:l³à?À!>ø?¡m:l³à?ç‹æ¹Ä®?Í:Q"#;?Ðè2ŒwÐ¥?Í:Q"#;?Ñïo'!‹t?Ñ[`®–€à?çH>ï:F?Ñ[`®–€à?à–ÄzN?ºôÔ9
ùÏ?ÞÒwñÿc?ºôÔ9
ùÏ?̔ã,ñ¶Í?µ>"ºÊ‡F?èÚÇ4ÒM?µ>"ºÊ‡F%MIXED4FGL J0914.5+6845?îÆÉ@	ì@BìÖÜGªÀ;ehžOÀ<ñ¼‡Û+4@! XÐ{®?÷#ք³ž?ÙúõÕÒó?Îf!‡+?ó–*C hÁ@Ãà`¨a^¿ã³!ž¶9¿êZ·D¥K¿èts¿ë<ú¿ÑUíýôâë?'Vä#'»»¿ë5tV2UNASNone?ïû¾Ù*di?9a–†ã?A›
Ú?9a–†ã?ïöŸøœ?RÖß}…
/?RÀäGgq?RÖß}…
/?ïÝ
»e­j?lFˆ^¸Žÿ?qy"h¦*Î?lFˆ^¸Žÿ?ïý_Ž}S4?"Þx␭?5‰ñ×Ӝ?"Þx␭?ïý
€°f?6êrú¿‹«?7«üñßè¯?6êrú¿‹«?ïÕ´6 G€?wµò1¤W?u%äÃÛ?wµò1¤W?ïÚ~¡Ï%Ë?xñt‹êò¹?rÀ¯
Bs?xñt‹êò¹?ïôÍv¸:'?PØèz'7?Ve!—^¿?PØèz'7AGN4FGL J0916.9+7756¿ìxö‹Y‡R@@åñà'Œ7À;ž«ôÌÀ=
àj8'þ@kg|×@v8äM?ËÝ
▸"¿µô<'x"ç?ækøÉ6@ͯö¨=¿ïyªæÈ÷U?ïý÷²S¤Ã¿å¼\aÕ²ú¿èL¶Ç§ÉÞ¿Ý}°6Ä¿Ð4'cšY2UNASNone?ïýÐO}?8GGpø7\?71}>ÒîY?8GGpø7\?ïñ;|¶gŽ?d€(ê¼ð3?]‰Ê*£E?d€(ê¼ð3?爛b)‹?†(ñT°JO?†Øgc%9,?†(ñT°JO?ïõ øÀh?A_Ž;¡?Uó¾kôp?A_Ž;¡?ïúÂñN.?D[!‡k£Ø?G"ô›‰ç?D[!‡k£Ø?ïª'ð£°c?˜l@nOÖç?…váb»I?˜l@nOÖç?ï}@ђ•€?Õ0:n?WåÊ=´?Õ0:n?ï"%uv?€ŠAÛï3è?‹6¼|3‡?€ŠAÛï3èAGN4FGL J0917.9-4755?ïB´‹ô{¤?ÀIܘÀ8ôIÐ-ª]À:À4¦Ð¹Á@P'˜÷@#9¾?ǾØWðVë?ÓéÄKd­@èñƒez®@e«…ÕA¿Ô0÷б^¿á§—Sn<¿êœ…ÂL@J¿èà"¿íÁ9¿ì?û}º@¿ïÿ""ÆUNASNone?æªjcdî?ÍVî]Z	?Ò«+96#ö?ÍVî]Z	?ãXÐê¿?́ {ág?ÙOÑú^*ƒ?́ {ág?ç6øuÙ1?³]™,²¹?ÑߒM?³]™,²¹?趩ÖcJ?ª:"½¡0ž?Í%X§êrÙ?ª:"½¡0ž?áWÛ~Kœ?ÒpSz%Šÿ?ÝPIhÉ?ÒpSz%Šÿ?·Îþ•Y´u?Ã|.{àÃq?í -G?Ã|.{àÃq?ÖÿގÒR?¶Æ~˜Ñ?ä€r¸–×?¶Æ~˜Ñ?´tí@~®?¤:d'
e?íqlB.´Ú?¤:d'
eMIXED4FGL J0919.3+6607¿ïþ2íN^@C¨ów[0À;$¬þÑ+×À<Ä +"I@ 5cqw'@V#£s7?ËöJŸ‹v?q$Ã-è?Ÿñvû4@ãæé¸l¿èòžm"׿à]àñFÿ™¿è@å¾5ZU¿ÎºE¡ô¿â}a?5¿ÛÂ;yRÒ5UNASNone3FGL J0919.4+6604?ïÿgkýˆ?ˆ®MiÂ?³Ý¿Þ7?ˆ®MiÂ?ï÷/Ó=k?Q¶ÎÎ,
?Q ZzI?Q¶ÎÎ,
?ïùNäRO?8@q†ŒŽ?JÄo•É?8@q†ŒŽ?ïûҙjt¾?%Ä.êNÛN?@µšE®èc?%Ä.êNÛN?ïÿƒqÌ(?ŒY¢›Í5?#¸Õc?ŒY¢›Í5?ï؅bÞz'?v>´<{e
?s½N‹?v>´<{e
?ïúÃ.'8C?YÞkô€¡?DóEÜ»Že?YÞkô€¡?ïíwÍAì?Rûo-ì—?bˆ3ç"C?Rûo-ì—AGN4FGL J0919.5-6203¿Ý`—ûõGÀ!tBÇû¬´À;,¥R4€:À<øðž³µ@u†6:y¤?üÅ㤧?Ò
 $Ð?è1³¡'œ'@ü™˜f"@8ªÄbC¿ïþ$}㰔?ïÿ5Ÿôým?ßnD¡o¦×¿Þ!ÂÝà›a¿ïÿ胸›¿ë©ââÔ?UNASNone?ägÌRð?Ës3 ¸¿?×0gËZË?Ës3 ¸¿?ãÊ!~LX–?Ìm¤ÚPª?Øk½gNÕ?Ìm¤ÚPª?â<§úk§ª?´¾3ª8J?ۆ°(°¬?´¾3ª8J?äJt¹¡ˆ?°ùAîä"?×kŒ¼ïé?°ùAîä"?Ñ—Ëýß?É÷÷ù?¥?ç|v´?É÷÷ù?¥?ʝî†
©??Ê,û¿16?éX"^|•°?Ê,û¿16?̦a¤Æځ?´šN¦OaF?èÖg–ÎI`?´šN¦OaF?Î%†,)~©?¶ØgÈï¦?èvžtõ V?¶ØgÈï¦MIXED4FGL J0924.1-5202c¿èŒš5Üìç¿ój
ÃödÀ9+ú—á2µÀ;#"i†¬@9ñ–°±
@C«»Û
?Ë®™Æe)¥?¿g­Ÿq0*?ôTÿ†]|³?ô(|P]?ïúI<‰ô
¿ã1T?v¿ìˆè6ú¿ãÓW€o|¿ïØjÅp·ù?é°â`‡ÕUNASNone3FGL J0923.8-5154?ïzü¤Å‹?¬˜m_Û? kluú!?¬˜m_Û?í$
ƒÿ²?¼cŠ¶IJ?·ߓq?¼cŠ¶IJ?íÔÂåmX?£r`+Q?·9YêŒcA?£r`+Q?íd²ÕˆeÈ?Ÿí£#^"?´ÚiT*Å>?Ÿí£#^"?î¹l9†?²Û'«r}?¤nI?×3î?²Û'«r}?×SZ΋F?Ó¼¸OÉ?äpÖR˜º]?Ó¼¸OÉ?ê<—²'žÄ?±ÉÂÇFmP?Ç
¡7a"ï?±ÉÂÇFmP?Õ`¨‰S?À Ov	òr?åO«¸;V~?À Ov	òr$MIXED4FGL J0926.1-5336?Û"™Wª`çÀ蚈¬âÀ:"hZ\lèÀ<P+žê;s@sCC¡•?ûŽ‡Lû‹?ҏ—U»?ç€ISQ·@
ͦ‹ðd@]aXµxÈ¿ïø|}ÿà ?ÁòSD¿À©çÚð&¿×°³Ü»Ø3¿ëþYl'à¿è¡a«ÃUNASNone?ìõ5JI>?¸(«X©|u?¸VWkõè?¸(«X©|u?쾞ý—×?¹È"Ç-.??ºAGÀ?¹È"Ç-.??ë	2´Éo?ª×ÀNúf?ÃÛ5-¼ÚD?ª×ÀNúf?ë¸ëÎDÇ?YVÔEÊ?ÁˆPÆìä?YVÔEÊ?ß5ş16?Ï<,Qö ?àe0g{å?Ï<,Qö ?á«@:O)?Ò
ÀÏàÊÓ?Ü©Í‹a¯?Ò
ÀÏàÊÓ?Ù%Š¹,?ÀŽåXi?ãm:£iüô?ÀŽåXi?áYlÏ¥Þæ?¹@Ôa¦?ÝM&`´B4?¹@Ôa¦MIXED4FGL J0928.3-2713?ç~gá³H@0úZxòZ%À;‹n]«­À<nÒæÂAY@ól¶6³E@w³•Ä"?dž<š«? ûéoð©?×=ÐE'Q~@càη]¥¿æLä_:£¿ã;¦i‹´Õ¿çš
¢ñ10¿ï÷Í⠜?ïŽÿªo«¿ïú#|ÜÊqUNASNone?ïÿy8aV˜?Dà•#'õ?ØøÁ7Hú?Dà•#'õ?ïò)'Z|?`ß͔¢«½?[ã®¸?`ß͔¢«½?ïáB¡)?t­Ù«y3Q?n꽙ð(â?t­Ù«y3Q?ïÿðl¨ä>ۘ"P,>ß&z´›É8>ۘ"P,?ïþñ¸?#Óˆ£È? äy+i'®?#Óˆ£È?ﯛcÄ«?(CÚº?"'4G"f?(CÚº?ïÙæhEZ?~0¿ÎR,?sËÇìv·?~0¿ÎR,?ïÿbûþ?"3'JEc?³¼Vž©?"3'JEcAGN4FGL J0928.4-5256?Êãt)Ù©e¿ötmZvnÀ:4^'Ӄ À;²'Œ6ڈ@!ÈÝ:Ùâ@%"ü|?ÝTd0V4¿Yõp7©?¨#¹ P5*@^
›h¿ê·'ƒû£?﹞âƒÃD¿Ü5b¸[ü€¿èìí¼0¿Åօˆ?ª¿Ô¨˜¥}ÓjUNASNone3FGL J0928.3-5255?ïøï¶9k?rŸ'äš"?LA'³(Ìl?rŸ'äš"?ïç£R2°?ul¿·^¨?hä\tßñ?ul¿·^¨?ï½tçLn²?šJ æý?€¢Æ='?šJ æý?ïðÇ9 CS?Mue­JŒ?^quAË$?Mue­JŒ?ïå	®?ehÛ˜!?jör4"A#?ehÛ˜!?ï2ê
­ñ?¬X¾àŠu¹?™¢¾FÒ@b?¬X¾àŠu¹?ï-;Îs|5?"Î߉N¸?šX†:'\?"Î߉N¸?ï¢a)nA?€HhE"´?‡gµš ë?€HhE"´AGN4FGL J0928.5+3916?Ú¦…1Ïþ@G:Á~ºñÀ;V›‡À<¼‰íT+Ñ@‹	ˆêË?ùÛR6-¹w?âÃ^YQªí?àyÇQc?õ
US«È@·r0É÷Z¿ë"ÿ*¿äÛibš)¿ØßüTyÕ¿ã|É´êWø¿ëáÂ]B¿ïÿž`¨·DUNASNone?ïù°-ï#?J7Šý3
?I?LU÷ãç?J7Šý3
?ïõù͝†?TG֏¸?TdÀ["¼?TG֏¸?ï5I/¨u?‰gås`«?™VÝ3+¹]?‰gås`«?ïñJP:"?EH3òUR§?]kǽr?EH3òUR§?ïñu-~"Y?`r½c'™=?]¥#Վ
?`r½c'™=?ïÖ%?ÄU?wl³ø䄄?tõívUh?wl³ø䄄?îÁ¯ÐâÜ?™lѵJí=?£å兇<?™lѵJí=?ïÙr²ÊÌ?do·›?sFýš<B?do·›AGN4FGL J0929.3-4110¿ïô~¾»«×@Û¼ôèuÀ;¡}‹QÀ<šÐüÝ5Ñ@$œþ0'~?÷´¿û-2h?Òj«ûØ?£bt"Q†0?ÐXÅ>
+ã@džaƒ}£¿ï½ÜÿõÄ?ïÿí@_Á‡¿ÞÚf]­[¿œt‡Äã|ð¿Ý³n!EÊå¿v"쩃iUNASNone?ïþÕSf?:ûÛ!?"®{p·aõ?:ûÛ!?ïå8p>Ñ?tâY
#j?jǏY¥fð?tâY
#j?ïèò@_ý¨?qáÒò?g
¿kÈH?qáÒò?ïøaSéu?Bnžò«È*?Nz°.y³	?Bnžò«È*?ïÿ![0?HªUÎÌË?ԜÇ%º?HªUÎÌË?ï1ò¾yË?¥õ‹•?™Á¨@ b"?¥õ‹•?ïîuÁ²¦?qÈØ
­?aŠ>ÛNš?qÈØ
­?ïßÃ]s‰Ì?j€éOù?pQ5
B?j€éOùAGN4FGL J0930.9-3030¿à/GÃãïÿ@.&?Ýe¡EÀ:àˆÛ—À<z á!¨@ ê
½,ñ¦?ÿ…˜Æ5?ÄPƒO*`¿z¾z~À21?»5y3'K?û1Åû!sî?ÖpÁÊoû¿ä ÜïYÀ¿åk¥€Âù¿ÖÓEA¨–ã¿Þ
`¨6j¿Ó_2•~'UNASNone?ïý‹eÆ¥¹?(IԔÍfM?3¤Ñ:ɽ?(IԔÍfM?ïéÍ"ªqP?hÙ·9·1?f2Ý|
P0?hÙ·9·1?ïõ7¼§2+?Bõ ­Š?U†±›ª&?Bõ ­Š?ïîá…¹à?Cºs±Ô?aäŒ$º?Cºs±Ô?ïý	Ç;?*@þ—Þû?3÷µßm‰Ö?*@þ—Þû?ï‡Ê9Ó?–LÚ2è•?Ž
q"\¦?–LÚ2è•?ïù#}'-î?Tà0º,–?Kr	ð%?Tà0º,–?ï¢Ï+‡ÿO?t'6Ô4'?‡L5±Xj?t'6Ô4'AGN4FGL J0931.4-3559?ïŸ%¹^A@&vT´:çÀ:ÉNÀ<\ø_»Q@  x"¦s?ú¿Íui8©?Ô¹CXr?Ò¦:&l{S?÷²åB˜@l©4:D?ïËM;5Á¿æ¾‹@hî¿Ú"Ø\¢î,¿Ýzz…\!¿ÞŒy¦Ž¿íò^ç1UNASNone?ï÷µ5Mâ?E ÉÀ$?P••è,ú2?E ÉÀ$?ïâlp¸ò?u>ȤáV¶?m"ôœt?u>ȤáV¶?ïÌU¹Îuø?vr'@§^'?yÕ#&ƒsÿ?vr'@§^'?ïädŽJ2?J	"#«?k›qÍX&?J	"#«?ïôÎìë-é?R&¶eë¶Ú?Vb&7bœ÷?R&¶eë¶Ú?ïD³Vë/u?¡¢5£¿§?—i•r§s?¡¢5£¿§?ïñSƒ¤?Šß®»d¦?Œ«)e´M?Šß®»d¦?ï§æǗ%?qvôäå1?†8[ئœ?qvôäå1AGN4FGL J0933.8-6232?ìB§øà…À¡2CI*ìÀ9þSW•éÀ<;<v¨Ô@­â˜»ù?ùï:µÞt?´=ÜÀ›ø*?æ&õ7O!¦@0M™gD²·?þ뮔¨n?ïçŸìš?¯GW™ˆ'?‡Æ¨½ÆA¿àµ¿äF¼¿îÚpžùÞ¿ïÿȽs"vUNASNone3FGL J0933.9-6232?^uz뭇h?c~·l§?ïðÅBg?c~·l§?±G<Ç´ô?°®™K!?í×fíäŽ?°®™K!?§dž{…Ñ?™Ú,åCï¢?î‡	¶&?™Ú,åCï¢?0ðax˜–ø?-1
}õÈ?ïýáô'ò?-1
}õÈ?l¨É#&K?mÏ°ÿÞ?ïãW6âY?mÏ°ÿÞ?…m~i¯Ÿ?‹¹[?ïªJfÿò?‹¹[?»Í&o¢ó?¨Æ#ñŒ?ì†[?R¢?¨Æ#ñŒ>µÔñùÈÖ>¾‡b8µ?ïÿýE‡ëê>¾‡b8µPSR4FGL J0934.5+7223?±1–¡Ç¯@BÏrÅz%À:Ð.ülÎÀ<–'õ@-ÄY`Ä@Œ½}¤p?Âê¹Ç·d0¿¤òåˆZ'?Û·pú¾øy@ûow‡ ¿á†XVÙ+¿æ潤:ÝL¿êžÔ6M™ç¿ê~"àÍ4Ò¿ßÜ»­?¿¿ïNŸË6öUNASNone?ïý¸†*T?@Ž«
1?2;Ï¥çÃ}?@Ž«
1?ïóåÄ%Ås?`¦¡3¨¹F?X4wã/Ê|?`¦¡3¨¹F?ïÊâ 	úo?y´ì'§H?zŽïþrd¶?y´ì'§H?ï÷{º5›m?<ÔÈø~?QŒ<­?<ÔÈø~?ïôž5hJJ?`Âk/Ýíù?V՝^ë¶?`Âk/Ýíù?ïÇg,ßÜõ?~ú܋ûÜ
?|Lis乶?~ú܋ûÜ
?ﴂ¸£íR?'œ¥@:?'ßQÊN"?'œ¥@:?žŒiþ?•¡ÔÉ?ŠVVH¤?•¡ÔÉAGN4FGL J0935.5+1152?¹t
0Ô¯@DÝ%þ—J4À;Öß3םáÀ<åCÖïe~@#^m"?ùÈÛ–ª?Ìù)a£3 ?cÕN?lì+@ÞM&yfs¿ïð®ôt±ƒ?ïìÐxR÷õ¿à5A` J¿ÖN0d¡À/¿è2D‹JK~?Õe÷áMRUNASNone?í1×U3Z˜?ѧQw/Ñ?¶qEU÷7Â?ѧQw/Ñ?ïóïyÜ 8?Y¨£¡R+?X!ÎÍP~?Y¨£¡R+?&ìÊ?ŽWWw,©¤?‡W6'$d?ŽWWw,©¤?ïõɼ«?FdîBô?UúlU†IÒ?FdîBô?ïú!¤É?Ve6¶®{÷?GÓz‡­ÿ?Ve6¶®{÷?ïЄVí"?y5pàø?w½ÿ;Ì?L?y5pàø?ï¨×$È	?ŒƒÁ_2x?…Ê6ÇÅÊ?ŒƒÁ_2x?ïÕ:ßò*?mL­>Em?ubõ‰×Ÿ,?mL­>EmAGN4FGL J0937.6-3358?éÌssó T@+&&ö¶À:Ä"À<6U¸™9"@®É"¾@tþ½	á*?Ãë"ÈÒc?–9;F8YÊ?Ò}y]9!?ýyðql©Ì?ïþ‹ Z›¿çš€'¿í.jÁ¿Ój¿ëíAÄÆn?°äÏÍÞѿɶnçi[8UNASNone?ïümX•dÎ?;Ä÷áCù?<•;B(|Ô?;Ä÷áCù?ïãgôå?wZ¥«\Lû?lb˜Á'ù?wZ¥«\Lû?ï´¹=mõ?}¤è¢ð ?'ѹ~ºèÃ?}¤è¢ð ?ïü*Nn^>?.È¢ÁY.?>­Ž:öɤ?.È¢ÁY.?ïÞpx¸ù[?v¢©£S?pÇÞ³Þa?v¢©£S?ï:ND«?¥ïÑNZ¹±?˜¶>>IÔÅ?¥ïÑNZ¹±?ïGo€Éò…?'Åå6¼?—æÁ¯Q?'Åå6¼?ïÇ`ߓÎÔ?uÞ&íyÈr?|OÌAû?uÞ&íyÈrAGN4FGL J0938.8+5155?Ã^zÊ  	@G>L/ƒ{JÀ;Wѹ›—¡À<ãÕçþ{@Å$ʏ°¸?ÿÚáb†?ʨ3PD¼?²z5?ÙJ?éwÇ·º@ã,€±¿å
f H	"¿ä©£1ÈÏè¿å˃á÷Vc¿Ý÷µƒ¯øV¿ÎíŠG?¿ïÿ÷Ò4ÛUNASNone?ïþ~‡ç·×?Õ½ŸiG÷?(e+Ù?Õ½ŸiG÷?ïöù˜Õñ?Rö§²?×?RΊ,ã?Rö§²?×?ïöÍÁ‹Èm?Dv³ûĀÔ?Rd}«µº?Dv³ûĀÔ?ïüF°úšw?%LŒÐú^?=Êz\nÔ?%LŒÐú^?ïÿ:¬½ýk?b½C?ªlڏ8¢?b½C?ïØ;Î7[?u›M¾AÌ+?sâäRzv?u›M¾AÌ+?ï÷øe	¢Ÿ?Zën£Î³ ?P5qO1µ?Zën£Î³ ?ïëƺ¹ú¸?X4¼*¬;´?d9E‡ýǍ?X4¼*¬;´AGN4FGL J0940.3-7610¿ïå­ó‡qÀ1sàGÓÔÀ9Ã(xÅ
¼À<'šÈÙ"@}ðpÀÝ@:a'ÑÖø?½=߉'æL?Øü
Ý©"ã@xØ앿ð@Kœâþ?¡Ë¸$Ê׿ÃÈ{ÄÇoÁ¿Ý1{"54¿æZ—ZúøY¿ïÿëJw¿Ø\:~6UNASNone3FGL J0940.6-7609?¶$±Hä¯?¿¤jG?í;i×iÊ?¿¤jG?ÞË*ÜÞ£ö?ɵè+aq?àšj'®?ɵè+aq?͹G˜ß¤/?³D"€©Sc?葮Èô?³D"€©Sc?ç'Û^Ç?­Wœ¥æÐ?ÑæÛÊIBr?­Wœ¥æÐ?"ì<äuF?…Þ"e÷,|?ï¬O&[?…Þ"e÷,|?·þZpÐ'?»·ÑÜÝ}?í<´ÍbÛ?»·ÑÜÝ}?˜£s÷™`+?Ž^ó®?ï:ä`ù¯?Ž^ó®?¿XJÏÆì?£'Ñ­"õ±?ìö¿#?£'Ñ­"õ±MIXED4FGL J0942.5+7620¿ï\=bX‡"@Aî‰v5çCÀ;ƒS¾ÃõŽÀ=MŽ(LO@ N
/-êõ?û]þ¸Ø#?Õ$¾!ŽE?ÝN']Šõ'@v?<Uñ¤@Ý]Ü)6/¿ïöK¶··'?ï÷
XH–r¿á³"6‹­H¿Î(ú »¿î™ð×n¿µË4*©øUNASNone?ïöáÿlÔ?Lô†Â1´$?R<cx…?Lô†Â1´$?ïìEÀÿd$?bWë%1У?cº>Þ?Äo?bWë%1У?ï&\yíF?'ø¥¢ú?Ÿ›4iãT?'ø¥¢ú?﬿Sðö€?h
¹½?"Ð+3Ü?h
¹½?ïã#VNô¸?nqy…Î?lÜ©ðDQ?nqy…Î?ï±a1¦É¶?"'"¶ä­?ƒ§³¦s¼L?"'"¶ä­?î›xC³‰?›Ùû¶#¥è?¦H{È7¼?›Ùû¶#¥è?î û¼_¨m?–ÚB\2E?¥ðD:y*?–ÚB\2EAGN4FGL J0943.6+4207¿ï'ÌFÑ0ñ@H"­}|,¡À;"‰"hØ1À<"5¬En@¿KŠíÚ9@H…ªÏL?Ñë¹÷Ýò?¿Y'A'+'?ï|ˆçš®m@—¨q£±K?ïË'`—¿èŒµ( 2¿åš'bEov¿ç,	þÜix¿ïÿÿ)@k*?ï™HÁ9ñ"UNASNone?ïþ"£Õ?l䧼X?-ÕÅ¢ög=?l䧼X?ï÷nIgZ¶?Rœ­Ÿ†Õ´?Q#lª™åN?Rœ­Ÿ†Õ´?ïÞnðΉ»?qð/Ôö?pȇšÊæS?qð/Ôö?ïüà\1ëF?%É]<Kvø?8ýèh?%É]<Kvø?ïÿÉzE?m¨ÿ¨Ž?
ºmA©p?m¨ÿ¨Ž?ïØÒ$Չ?wsÇ=çÐ?s–òûS« ?wsÇ=çÐ?ïь)?|RÑé¬(€?w9ë"V#?|RÑé¬(€?ïí²Šx¶Â?T³Ë;#k?bMu±äeY?T³Ë;#kAGN4FGL J0944.6+5729?îÉ75:8O@F¹‰ßrïÀ;Õ09ƒ¯MÀ='¹@ ۑ×-xß?ÿœPbîâ¡?Ñè[ôrƒ?'ÅiV/âq?¶¥ŒÁïÏ?ý§gıË?çD ¾{ü%¿ãøÃ*Œ›"¿åϙ/çNX¿Þ§¨ìMñ¿à¡¿}ƒäQ¿Þ73ÞSÝÎUNASNone?ïþ?ôÀ9t?#éUZE!?,²ëºòÕ?#éUZE!?ïôÉ`å%½?U|dS3}4?Vm=ë|÷?U|dS3}4?ïôšð™í?Zæh·Fü/?VËáߓVê?Zæh·Fü/?ïï\ûiÔk?CIV˜ú?`£VòÅ ?CIV˜ú?ïþâ˜)ñ°?\R³¾?!Ö}Ú³¥?\R³¾?ïÒ¹ÂHH?v
ŸØ§fV?v£ÔߜY?v
ŸØ§fV?ïø:c~Ä?`øݔu¹?O¾)©
?`øݔu¹?虜Sõ±¯?uv®©p±?†ÒjøDÀf?uv®©p±AGN4FGL J0944.7-5124?ë¾÷!F?övaÍ
àÀ:xÙÔLgÀ<»få@ Ú¤.™p?ý{ÛB±U?ћ)Q2!»?ÏîƒUà\L@S_2•?ý%'6¥®{¿âšÆÀCQŽ?ïÅ2¤—ú]?Òë@Ö3ÿ¿ØîŒÛE5"¿âù́'²Ì¿à¹ë^2eXUNASNone?ïî`ëÓ"Q?dîª²U?aŸ	!¾Î?dîª²U?ïPû Æñ?œá6B/›?•àœëç!ë?œá6B/›?︷KR±?~;Òzžõ)?Ò-7d ?~;Òzžõ)?ï$æk?ŠZÝ'U?Ÿ;Hd¼¦?ŠZÝ'U?ïØT6Qåj?pÿÇÐ?sÕäâ»÷?pÿÇÐ?ë-»P½K"?Æ=Þîô{#?ÃI½
ѯ?Æ=Þîô{#?îZ4ôÿEñ? CØ`Ã~?ª\°´W#í? CØ`Ã~?ëÜi•oéG?¦Or \U'?ÀŽYª@Zä?¦Or \U'AGN4FGL J0947.0-3548¿ß××C›ý@+ˆ7q†UÀ9øúÒ¶À<óähÊÅ@FjpŒ/#@\0LÎå¬?Å=ê†Ç?áÇV +à@ìxc¾ì9@œI1wF^?ï«<ú\R¿à±%q©ˆ¿éñ&³ÈïÈ¿ïÿÿ" 5•?ïʧ߭z¿¦:ÌbLXýUNASNone?ïM
É¡c?±Ïdwr?–^¦Ðû	ë?±Ïdwr?ínÖË0óñ?Ã!s|=W?´‰I¤Ržø?Ã!s|=W?êÒ-âï×q?«iäEöj'?Ä·Ht@¢:?«iäEöj'?ïó‰sL?Y÷¢B?XäìòeÇ]?Y÷¢B?ìl6ñ?ÁÑóìæ§?¿ÜžHw_?ÁÑóìæ§?×ÐˣƳ?Õsº$²¡?äuš.§?Õsº$²¡?臏´ú"Q?¶;}¸@Ò?ÍáÁ,î»?¶;}¸@Ò?ílk+O"?·‹gÄã´?´œ¦¤8å?·‹gÄã´MIXED4FGL J0947.8-4234?í¨ÓsZ@ þØôù;ÁÀ:[=~HÀ;ý57ð1V@¶ P¢@°cûRV?ËOÿÇ é?Åëq¾cÒ?úÂ(]í@Σ'•¿Û¡ßyw»¿Ã³œd¥-¿å]&¡ª_:¿äÞ?:þ¿éð9¹_2¿ïÿØ}ZÙUNASNone?ïë°wN ?_ç7¯?dOˆ­ÓØC?_ç7¯?ïÕò&'TÆ?{ÖÁ™$ð?uì­6µA?{ÖÁ™$ð?ïÇFtO ?sd¿ÛjNô?|\ŕ+cò?sd¿ÛjNô?ïÜof·'t?Pé®ÿmÅ?qÈL‰jRQ?Pé®ÿmÅ?ï"ÄCË?‡Þ§&&?ŽÎþk°q/?‡Þ§&&?î´eÑ|E1?«¬3JìH¤?¤¹¢éózì?«¬3JìH¤?í"ó}™<?¥ðܔž­?³~èd)£?¥ðܔž­?îø¨Šo§z?ˆ:÷§à¼ë? uwU•ìb?ˆ:÷§à¼ëAGN4FGL J0948.0-3859¿ÓüŒ-râ@&y*Qã!£À:¶¾(Å(À<£hOt²@›"j8-@A³ÿvmE?ג¥^žÆÕ?êÅÂíOú@'ë¾íç?þ õ;5?ç÷X[á¨&¿ÝñÆ@ì"M¿ìþ£^"_ô¿ïÿ'ãñ?ïø¼ßï¿@¿ïûÂ-·sUNASNone?~:î?ÔÊ+¹•ƒ?Ž8ݨk?ÔÊ+¹•ƒ?î*‹;Ta?»¿%•÷ß±?®}WJ'ëî?»¿%•÷ß±?í¤¸‹Õ?"ë)»,•?²Ûò:·ºV?"ë)»,•?ïäá°Öï]?hµ,aMÈï?kNòãe?hµ,aMÈï?íL®n˜?» UÒ
:?µŸÚŒ!7½?» UÒ
:?ÚãíÈs'?Õôò™Ç%?âŽ	÷F7?Õôò™Ç%?猥Èڂ?µ6äfÉ?ÑÞæ´nJû?µ6äfÉ?ë"*]»`Ø?ÁNù¢Ã¹Ô?Á¯V‰|ž?ÁNù¢Ã¹ÔMIXED4FGL J0949.8+7551¿î61yc‡ÿ@B?ÖbwÄ]À:îJÔ9¨˜À<ÚµŠè@ø™Iè^?ÿj~…A?έ©MÙ?Ó¦¿òɶ˜@¡/à˜[¬@‹¸Þ6¿ë¸Á>#Q¿ÉÿÓµI¿àÃ.ô	Q¸¿ä ¶© ¿èae`,¨¿ïÿõƒ¥;ŽUNASNone3FGL J0950.4+7550?ïôƒÓ'Ai?Q`œ͆-?VøYYîÌç?Q`œ͆-?ï審À?fyhƒ$?jPV}¼Î?fyhƒ$?ïŸS¶q§É?}Nf•°?ˆ+c–
¯?}Nf•°?ïœuíu—d?g|z,G'à?ˆâ"©y^Ü?g|z,G'à?ïÎåú¬j=?}Qn1 ]?xˆe?}Qn1 ]?ïÝÄì¯?‹	Wê
)¨?Œ¾"vi?‹	Wê
)¨?î7îMd!? ›9—Pi$?¬(½rï? ›9—Pi$?íöu5>Ù¸?•iØ ò?°LVSãpÂ?•iØ òAGN4FGL J0951.8-3711¿éØ?ì¡uÓ@*-À3aVÀ:µž·æ‹»À<:îí‰@AÜ¢òô@¯BÇ$í?Ö9íAat9?î~;¹ÿk@>l`{jÚ@3ô–#î¿ìÏj¡^‰ù?¢Âæo
Nã¿ìà=lòò¿çí?3¶?¿ïüBK?ïęAÚëÉUNASNone2FGL J0952.7-3717?îEp³­}?»qþãë?§ë¨õ¡+?»qþãë?ìðt•pâ?¿Q%ó¬Ï?¸|_{Âll?¿Q%ó¬Ï?ì³þþ*ñ?¦úçm[#ò?¿B`¨v?¦úçm[#ò?î†ÄÒú±?"¹zT?§ŸÃ´ˆ"ó?"¹zT?ꕋÅÙq?Ç8ËКÚ?Å©ÑÈèš;?Ç8ËКÚ?ÓNíX?Ò?æÓfÍ?æX¹	vvT?Ò?æÓfÍ?ä>nÓSh?¶fIöÎ
?׃#þYY/?¶fIöÎ
?ÝÁ#K^£$?ÁãÏj-gº?ánZP®n?ÁãÏj-gºMIXED4FGL J0953.6-1509?ê×I"¼K(@=šO—íÇïÀ9Î,UÉ`1À<ˆ¢Ù´;Ü@"²U}5
?ú»	 :2+?ºžolIP?å(U{\˜@%%"1zÌ@9RIMü¸¿í<Lû[V?æžÞ&'d¿ÉMgfìs¿æ	s˜Ôx¿î"žã…uö¿ïûÌßÂðUNASNone3FGL J0953.7-1510?'¦ª¿ªÒ?¤Í5Öł?ïrʩ˯°?¤Í5Öł?ÅxܪæH?Á£×wÂüŒ?ê¡ÈÕFmù?Á£×wÂüŒ?º6¸Šä?¦ÝÍæ}M?ì¹(î¿C€?¦ÝÍæ}M?—»ýe?†ö.aã¯?ïCz''P?†ö.aã¯?—±œ'¢¿?¿…ÛTW¤?ïBsøÑZ?¿…ÛTW¤?¦ð:–ýþ‹?¥ý|KÒÚ?îüVt£7?¥ý|KÒÚ?•ßš.êÏ?FóùDK ?ïQ.CñX?FóùDK ?AÕ8…®ïí?8[W"»?ïûŠ±¹ï?8[W"»PSR4FGL J0955.8-4106?ép ¾*al@%ì|•|ÔÀ:@\78{rÀ;¼$·om@ÙÜ»W@z[ñ?ÑsÓÜí?â*8ÅC@Þ¦c¬wÃ@]!)ÆM¿Õ§ÕÜëÓοàøi"®U¾¿êû/—@ú¿ïÿò(¦è7?Ѩ©ï?çjNRsjUNASNone?ïõ'é§#?\yƒ:'?TÚ,Ò¶»?\yƒ:'?ïl¶[¾?£2á¿"?E?'i4"¾‹?£2á¿"?E?î…OLïFõ?— L¼N»?§«3ŸE©?— L¼N»?ïöǂ¾"X?L›hmÝÉì?RpúN?i?L›hmÝÉì?ïÜÑúU"}?ƒÈûõ˜?q—î£]|?ƒÈûõ˜?äÃÍìÿ¿‹?ӗæJT"?Öxd&€ë?ӗæJT"?ëfp*?®.í‹?Ãæf?W·?®.í‹?î/%žuF?¬ƒ):—ó«?­
¦ÌÄ ?¬ƒ):—ó«AGN4FGL J0957.3-3851?ëóÏ^ç0@(ú˧2ßPÀ:sö•3À;í┵.K@¬Þ½e&@—s\.Ë?Ñ+^×{Ò?Ó
©`áí?ü%F
¦L?ö—‰çtî¿¿ÞqOÎtm¿ä[Ò>%Õ}¿í»ñ³6"Ò¿â'¢;(Êú¿î»Oag#%¿ïÞú̺XVUNASNone?ïxš²?¥<­KÑZh?Þpçˆ_Á?¥<­KÑZh?ì33‰o?À(³ùþDz?¿öfc·4Š?À(³ùþDz?íð}»"×?œâ¡ÂªVx?°|&"F?œâ¡ÂªVx?íê«LŸjê?"Z=Xé	Ë?°ª¥š(Á²?"Z=Xé	Ë?í¥'Ï?²Þq3ÇY?²×/ì]µ?²Þq3ÇY?Õï*[Y~2?Ò]Ù¶%|¢?åjÒS@ç?Ò]Ù¶%|¢?çõmÇ?¸º9Cºâ?ÐÚáý$r?¸º9Cºâ?Øpmc¹@‡?½m^õ{9)?ãÇÉN#_½?½m^õ{9)MIXED4FGL J0957.6-3051?ì6ÞãÈd@2µ,'¦77À;(Òü'¶vÀ<šˆÉg½~@nןc³@9lÅûø4?ցùje?ì)KRä©b@
´¡\Üyé@re"C¡À¿æR:Ê×)G¿Ö™}j¿æt5ýö¿ïû©žõN ?éŸ@¤Šä?çÂ)óUNASNone?ï«c)´É?'Iu"×'ù?…'5'ͼP?'Iu"×'ù?îøŒýc?³@%)È4é? Ç?×÷Ç?³@%)È4é?ívB›W–?Ÿÿ¿Éþ?´Më(—Ê?Ÿÿ¿Éþ?ïôëӉe«?Um$Ññ"?V(XúóË?Um$Ññ"?îã#+[Öô?©´ƒP"&Ÿ?¡ÍÍJBÁ?©´ƒP"&Ÿ?áhï¶9k?ÕzÙZNÕü?Ýé. "*?ÕzÙZNÕü?äÑ.Š›¾§?¹¿›-dßu?Ö]¢êȂ³?¹¿›-dßu?íšT¯Q3F?µh	:d ?³-Z…äYQ?µh	:d AGN4FGL J0957.6-5208?²ÑÇQp‡"@ɤ^ïÀ:€<_+߂À;Ï _Š@è°XÍÌ|@X¢t3¯?Êm§"n>ø?±´p	¨Ja?æͳaÁ»ø@Xœsé†Â¿î;Ɵâ?ïöÌD琝¿áãñâ0a¿é+ñUBQ´¿å"†ŸìÄå¿à—|ÞÍÖ7UNASNone?ïýöœ:D?GÁCš=_?0K·P8Ó?GÁCš=_?ïâBӗÊÀ?{	SÀŽQ?m½,•¶?{	SÀŽQ?ïÜ,5èð?t½»Ž–C>?qéå‡ó?t½»Ž–C>?ïøû~æåÓ?5ÙÊñB§?L¦a4ð?5ÙÊñB§?ïùIŽOŸ·?KÖ×øO?JÙÅùñp?KÖ×øO?î¶Ks›Ù?³h®C ›i?¤›HÈÖ$
?³h®C ›i?ï?9•'¼?ÿbŽO?‹ð1"¼Y?ÿbŽO?ïÖó6}ï?h£ÌWç~?t†dòÁ¨ª?h£ÌWç~AGN4FGL J0957.7-3510¿ïá_ŧ-@.Οð˯–À:svð!fÀ<(˯–[!@Rqé&t´@!Mryš ?×Ëq'úä?áƧ"=çÂ@	o!öÊÍ?ÿÅäÆh¯—?ïú²]à°Ú¿æˆ(Øîn¿êædþ²M¿ï†Ä);
?æûÎRÞÊ¿¹ŒÔ_":UNASNone?ïää´R¶?žäُ¼í?kKí♯?žäُ¼í?ï
MÊç?«#j'Žö?œVYk?«#j'Žö?í'­9V?£B ‰X÷?³oŠ–£C\?£B ‰X÷?ïçx…Þâà?clNÜSÌà?h‡z@h
?clNÜSÌà?ï0;Æn}¦?©—sg•`[?™ø‡5Ÿç??©—sg•`[?ãÏaýv
?Ôâ
X«›?Ùða<æ?Ôâ
X«›?é"œY½a?¶H?A«?Ë孎™
~?¶H?A«?ë!
 aÁ³?Á^T…Nš(?Ã{×~xù2?Á^T…Nš(AGN4FGL J0958.6-0522?æ, s—@=@BŒ>§¼À;"žõ#-,À<›w3=D.@ØZ°O¾"@²¾‰¬½?Â9q{BkŠ¿±"Žg·IX?í1išÐ?ù͙Ëî€|?Åû`ž{U·¿â;}^ûc
¿ìúþ£ßm¹?ÙÈuO7u¸¿â¥ýzïð8w?Ò~UNASNone?ïû˜P³¦?7g¤@Éï,?Až¾ &†?7g¤@Éï,?ïãþRçêœ?rzÁYŒÎ?l­—Dq?rzÁYŒÎ?ïáW9¦?p"™À
R?n¨býS¼æ?p"™À
R?ïå¬ö©Ñ0?U´f
ö?jS	')ÏS?U´f
ö?ïí[ÙMAZ?]§ô^_|?b¤&¼]Ž?]§ô^_|?/Õ}?"Ñø?H=§?Š"ôïŽ3?"Ñø?H=§?ïÚw$àÆ?w©v#"dô?rðDs¾èÚ?w©v#"dô?ïuMƒ?'!'q3?žq\§!°?'!'q3AGN4FGL J0959.1-6441¿ïâœU>S€ÀâDÀú0³À:˜8±ø50À<§÷*ni@Á¥"Ò@-IÿþR?Ðô«£‡Y%?Î"øþYà?ý·}°/@¹‡!m¿Ývz"ð¿ç—ØÏ9Ž—¿çW\¨w'î¿ÞГásÍØ¿ïÿýF\I¿ïƒY¡\ºUNASNone?ï֟)⍺?qÃg€e>?t°kˆ–½?qÃg€e>?ïßÛÞ@EH?vPÿæAu?pùúcÓ?vPÿæAu?ï¤_Ĝã·?«4'U?†èߦJ*?«4'U?ïÚÙZq2?U<áj87?rü"q³âË?U<áj87?ᅧàKã6?|
ù7,¢?€G÷­üs?|
ù7,¢?ïR.¬2E?£ªØug?•¼z/¡![?£ªØug?íõ›q¤Í?£"?zQEf?±âS#(ÿ?£"?zQEf?îÚR,ì•?Ž›ÁÎ'Q?¢Zß}16·?Ž›ÁÎ'QAGN4FGL J0959.1+5719?ÕßÆcú@G¥"À%À;b,µj°À<"φ»p"@‡Ž6¼@ÂzÞÃo?Ã)2(q8R¿¶ï.vŠ÷?ô`­¤éXõ@6á¿Î¼?ÁqËýTª¿êB±(+˜¿çc˜UÌ»¿ëõÖEòR˜?ØÓ P—ó¿ïþ±¶ÆÑ
UNASNone?îãµ"pµ?·ճ•(?¡Ä­Ü&¯?·ճ•(?ïõl¼tm™?UÃñÍ[i½?U&†ÇmÞô?UÃñÍ[i½?ï³['†?…" ź+?ƒ8©EZfw?…" ź+?ïþ|g7O?%ÊÕÚE8ø?.È9Å·½'?%ÊÕÚE8ø?ïïÔkª?eB¹H@¢'?`û+è5½ã?eB¹H@¢'?ïÈL¬DÛÁ?{í誾¥?{٩ۂ[ˆ?{í誾¥?ï/U¶žk?Œ–8Ù:?‹ô*"™õc?Œ–8Ù:?ïÒó>Èßû?w¸q
òр?v†`'BÀ?w¸q
òрAGN4FGL J1001.3-2040?ſtP{1h@:ê7&úÆÀ;LÇ+£ùÀ<½oe©P@ ŠUŽ¡™?õL«	-¦+?áÀá?µ"?ã…ߨq£±@tœŠâ?ôÜþ(º¿ëì&ďç?ÐݧESÇ'?ïÅTӖëi¿¸ÜÐ{)Ñ¿æ—IÈ î"¿ïÿÿ" 5•UNASNone?ïñÖ͐?\-{G§ê?]ÀSªê[?\-{G§ê?îo&ÂÈ£?±0ÔE}?©–g*Ê?±0ÔE}?ï^©Ü1ï'?Šu`?"*Ä~éwÐ?Šu`?옜'ñÑ-?ŸÅâ_̒l?»;èqv˜?ŸÅâ_̒l?ïéõ:Zè?cí|¥?f
Å`†ÐW?cí|¥?뒫•çÕ´?Èe»ïbˆ?ÁµQ¨`©0?Èe»ïbˆ?ïA-ìıB?'e÷ü\?—ÚBl'A¿?'e÷ü\?è¿·u)?·ŠÅF×»ú?Í"+›[³?·ŠÅF×»úAGN4FGL J1002.3-2810?ëŸ\¼!7@5k»ƒÏ,ùÀ:әt°¬À<<íÜçÍ@n݃S\@!]³9}Ð?çÓÌ@
>?íU/<-­¸@¦ó|cþ­?ó-ƒ«ñŠò?ïö%÷
ø¿ß¸ç¨eÝ¿ìuL}‡\¿áó{jª¿ï÷dP±¿ïüK_ÏÉVUNASNone3FGL J1002.0-2837?ìãD™ž2l?ùnze?¸åÛ4XG ?ùnze?ع*Yè?Ñd™€í?ã£ðêÓ?Ñd™€í?ìjc<ª2?¤Zñ쀗 ?¼¬æ¯6m?¤Zñ쀗 ?»ÍL=_å?¨þ™XÄ Þ?ì†VxT?¨þ™XÄ Þ?è· ˆK=–?ÎC&
Žf"?Í!}ÞÓ	¨?ÎC&
Žf"?¸XgB€ïY?ÂÔ÷da9½?ìôóË^õ?ÂÔ÷da9½?èEž.B¢V?±òš¾¸E?Îé‡Fõv©?±òš¾¸E?]u\ÚÏ&?[0H'Øï¢?ïñEQ7è?[0H'Øï¢MIXED4FGL J1003.7+7049?½½úü#ì2@D4cŠ	À;Ä5LèæßÀ<ÝrÐ×ôH@ ñc='Ó@
&ˆó?ÄÐR¾=èÄ¿·é¥´¦?퉎;Tj@³sŠfK¿åV'""F¿ç5:	Iú¿çú+	™ö¿êø¥˜«]?ÊÃgÉ<õT¿à•½ÀƒUNASNone?ïþ,쥸¿?"×(>²kc?-13‹ä@§?"×(>²kc?ïöâyÔ¤ª?Rv~¤…6ß?R;¿*ˤ?Rv~¤…6ß?ïﳙÊìÎ?_¾ôчt?`Lf	2t?_¾ôчt?ïþ´€ÐŸë?äÑg:Á?$·óÔ@‰?äÑg:Á?ïüsÀ/õ*?8َt$Ü_?<aý†¿Þ@?8َt$Ü_?ïՍÓM?u£d'a¡?u9~þmÉ?u£d'a¡?ïñ»ÆrÉ?h›òÀ?]̈–Ö]}?h›òÀ?ïìLÓSŠÓ?e<ùO ã?c³,›÷
Y?e<ùO ãAGN4FGL J1004.6-5215¿èê)T@5+Z÷[À;"÷8±!vÀ<‰E=÷²T@î­94?ÿ÷i=±;w?×RaA
'c?éÚÝfx@¥ߙX@|´>
§¤¿ä9Œ~($?ïøٛhÞ¿Ô¹+ºîÓÞ¿Ýq׳°œ¿ïÖèå1G¡¿ïWîÕSUNASNone3FGL J1003.7-5215?ï¾xK@E?œVäk¹‡W?Ÿ(0ýw/O?œVäk¹‡W?ìpóã¼þ?¼A¬Ž=ñ?¼ˆ`â?¼A¬Ž=ñ?î¢=#™Z?™'>
ç4Ž?®uÜ2í`?™'>
ç4Ž?ì1¬aŒ%×?›_—ŸU¤?¾rœóžÑE?›_—ŸU¤?벑•Ç°Œ?¸z=j¼ò?Á5¹¨á=Ñ?¸z=j¼ò?ác¬F^M?Ò0'…¬?Ý8§sCeþ?Ò0'…¬?çÇS?¸€Ú¡?ÐqYÉõ×Þ?¸€Ú¡?àºG™Wç?¹µ1ÿÆ8"?ދùpÍP3?¹µ1ÿÆ8"AGN4FGL J1004.8-5250¿î?Ä!hÂ@—a_–iÀ;9
ÏÌ[ŽÀ<X·Q:…@$Þ.ŒÛE6?ø†Ì7{—P?Ňϗ­[B¿·¸ËŸ6wÇ?ù¡cýÖZ@JÒ1e©¿ïÿ˜f"²Ð?ïÿõ^'¿¸œmŒ?¿éf è¿äj&¯—1à?Ê[å™w_ÞUNASNone?ïþÞ/©CŽ?!"…	‹-Œ?"	"¶;Š?!"…	‹-Œ?ï¼	µØ¶Ý?••UÞ¸?€ý'Œ'ø«?••UÞ¸?ïË/coæî?€š›íÉ×?zhNB)-?€š›íÉ×?ïá
T,?gØE£.Ã?nõçÊqH?gØE£.Ã?ïþBIÀW7?/Áص®‹?+Ûc¿,ã¹?/Áص®‹?í¿Ê\sã?ºü¸
`ï?²­…U?ºü¸
`ï?ï‹ÉQ(x?Û‡ï…Ûã?:¼ãíó?Û‡ï…Ûã?ï0Á¢æä?—8·—á|•?™ç˝ü‡?—8·—á|•AGN4FGL J1005.5-5708c?äTÂÅÀq¨¿ór˜Ù€9vÀ8ùáy,;ÈÀ:s™LlÀ@<½J£½@7­eÿ8Z?Ê»˜Ý\#?ã·¦±.@ö£ð4±@ðbF¿íÖ®b~zY?é0ðÎ3Õ¿çñûûŽ8¿ìài·ª¿ïþ݋`ñ²¿ãÙ}'ÕUNASNone?Ú9úÿŽý?ÑK±P¼Ó?âãü8?ÑK±P¼Ó?ÉA6~Iæ?ÂeÉ6Ùõ™?鯾²`m‡?ÂeÉ6Ùõ™?âGý@÷°À?µ¸°÷h´?Ûp~ž€?µ¸°÷h´?Ôý¶‡žð?²²?­?å$þ<0ˆ?²²?­?ɋ{d¶t,?˸d_ûé?é!&Òbõ?˸d_ûé?Œh;"¢?ŽJlà¨÷°?¢(¶?ŽJlà¨÷°?Äґ¹6©?°˜›ßrÐ?êË['²U¹?°˜›ßrÐ?€°+²-Š¸?qۗûÒÏ?ï½?Q,K?qۗûÒÏ,MIXED4FGL J1006.9-2806?îѯ¨#Ë@6!>‰¨‹À;=Õ¾
iÀ<m7Žâ†r@ÅñÞ&Ò@™þ†ƒ<`?Ì™<§{/?'ÑŠægAq?̃ÛÂ3@‹µ`£¯?ïåe¶™…?ì†e	o‹¿ì£é~´;¿Ø%}}":7¿Üøe-×)¿ïþ´ -UNASNone?ïõî}1ë?'ߦ,õ¸q?T#‹«ªs?'ߦ,õ¸q?ïçY³z–I?sgÊ$Šþ"?h¦LeÍNÿ?sgÊ$Šþ"?ïÌ·ä»ßr?z,šƒŸ•[?y¤
¿œê²?z,šƒŸ•[?ïí'ÖS?L9ND¤?bçØÝJu$?L9ND¤?ï㵘K€?pI7"MÍ?lJåïÐ(?pI7"MÍ?蠟	Øi?™
Ó
%3E?†Ö=¬uÐ?™
Ó
%3E?Óikv?‹Å\¨èæ
?ŽSË)¾?‹Å\¨èæ
?ï…ID[hu?'Τ'8?Ž­®Þ×»?'Τ'8AGN4FGL J1007.8-4514?ΞÅÄVô@!>—Ðk½¾À;^(Àª'À<p‹â÷±}@!ö¤Q-š?þù²©5?ÆÛK•ª¡ª¿²ˆœFG7!?óõ«é'v@vä;ÿ4©¿Ó¬ž"Í¿áw™:¿ê®ßa$F¿ïÏüE±?îüwµCCL¿ÒP|VUNASNone?ïÿ$Å ó?$®rÿÚ?gWOÜÕ-?$®rÿÚ?ïæÁÍë/ä?vÚyȕÉ?i>1ú³Û?vÚyȕÉ?ïµöá7+Õ?'Kª ÇÃ?''G¢¾ÌÓ?'Kª ÇÃ?ïÿ¼&‰Ï?{݆lˆ¥?öIšRÐ?{݆lˆ¥?ïù±Árj?RæpÕZ°ë?K8¹ä
?RæpÕZ°ë?ï&Þ²}k?¦A´°jNO?›0)°R™?¦A´°jNO?ïŠtÀ̃?Œü»åºR£?bÐ	O;?Œü»åºR£?ïù[)W£f?Uq¬Àêͳ?J"Z¥KË?Uq¬ÀêͳAGN4FGL J1008.2-1000?åzñ+¤Ò@AߥÁƍÀ:7äÞ;ŠÀ<PP¿54•@ãá5E@)ªIë?Ãb'Z/÷??µvÄ­n§?ëýdQµ@gõ†Tmk¿Ø³D›:ƒŠ¿èfœK›à¿í|KÀrÌP¿åï`«;'¿ï÷¶O²Å»¿îʇB'UNASNone?ïö?:00'?[3ÐÓFØd?S‹!'ç?[3ÐÓFØd?ïâ4'ñÉJ?{@`ÐGÔ?mËm×<õü?{@`ÐGÔ?﬷ճ•?Šÿ/È?"Ò
 Ù.#?Šÿ/È?ïײë
‹°?a촅˜"À?t&Šfî?a촅˜"À?ïޗø&9G?u"·1#s?p´Òhš?u"·1#s?ïm Uq1Ø?¡8›â¥?'[õQÙÅ?¡8›â¥?ï‰Ìë^:ü?JÎî*¹"?ŒÅ%¤í?JÎî*¹"?îQؗÜ*8?œêª¹®`?ªâvƒõ*?œêª¹®`AGN4FGL J1009.5-0034¿ï.­+`›@Eß;dZÀ; ¯7'À<ˆ©í¤³©@Þ@ÌùÃP@RpEy‹?ÔÅ$'n|?Ô­ÎÚÄU?û¦y–ÄÓ@
›Ž¹¿ïÿŸ‡ð#ê?ïõ}€3l¿Ý ó*.§³¿ç¦Æþ¬˜Ð¿ãmZ@¾61¿íÚï9ßßUNASNone?ïï'"þá-?`q"!L¯E?`ØkÝbâô?`q"!L¯E?ï×NIJ]?yQÞÛGWæ?tXÛZÑ1?yQÞÛGWæ?ïn'(±Ž?…{99æf?'/ºäµ$N?…{99æf?ï¡wVx²™?jÚ´–õûD?‡¢*l"- ?jÚ´–õûD?ïåz¿Óƒå?ex±Î3÷?j…@0›£?ex±Î3÷?ïAmŠšÎ?¡ 	.Ä¿?—Ò\®¬¦<?¡ 	.Ä¿?îâ˜Õ¾&Û?–coÙmß?¡Ör¥Õ`F?–coÙmß?íÎ'Ëÿzý?›£‹Ÿx.?±ŽÁ¡N'?›£‹Ÿx.AGN4FGL J1010.0+1416¿ìPÚÁŠ¬õ@I*û~ÿ—À:ëG‰+MÀ<eÝãu…¾@¬¸§{Úl@L®ì?Á¸#G'Ëw¿»wۃÉΖ?ø†!Ðý?ö…ÓÉÁ)«?éÛÁÝ/›¿èî÷ßËF¿íŽÌKD¿Ç³A¶X¿Ñ(}ãǐ¿ïÿ^º z^UNASNone?ïôŒtˌŽ?ig–¬#?Vç òÊ?ig–¬#?ïFj§,˜ÿ?¥ÃS܈òü?—2«¨)?¥ÃS܈òü?ï}+¼hÈä?ŒU}'ŒÑ?Zˆtž±ˆ?ŒU}'ŒÑ?ïÜG1Jƒe?dpWLê?qÜgSßÉ?dpWLê?ïæ‡ÀB»?p·µÕƒb?ix?ðÆ}.?p·µÕƒb?èÆ5ûם?Ìs[4Œ­+?Ìç(€¡Œ?Ìs[4Œ­+?ï*eÈlüê?•9Œ»%4·?š³Fë*Ó?•9Œ»%4·?ì÷Z"RW?±Œ""'b?¸E+ß%Ã?±Œ""'bAGN4FGL J1011.4-5729c?ïýÁìôàg¿ð¡ÒM?MôÀ8ÁÚWÏÊ®À:Fá$r¦@kŸ~Šõg@b¡ Ï?͹§@¡/æ?ÖK2»"@÷ñsuB¢@|{ðȀ?ÛªcÇOµ?ÈTZŠ»x¿ç½¾a¥"¿é¿*þ~ð¿ïò-DéN?îK®UNASNone?ç!
Ýåµ?ÑÞ6JنÞ?ѽêD4•ç?ÑÞ6JنÞ?遧¬E²?Æhðà¹yð?ÉùaNé5þ?Æhðà¹yð?⪩¾Í'2?¸2RBÛs?Úª¬'e±œ?¸2RBÛs?颦gL.F?°"¢ñãÛÓ?ÉufbÏFé?°"¢ñãÛÓ?à4E"ƒ?Îmd¡.'J?ߗéuúØú?Îmd¡.'J?ÐJØ	°œ¯?Ðãpëig?çړû'±¨?Ðãpëig?Ó"@$eîz?»A	[¸?ænßíÍÃ?»A	[¸?½Òþ¦?¯
ÔF-©?ìE§œ+??¯
ÔF-©,MIXED4FGL J1014.6+6126¿¤ëŽðþmI@Gsý'w>%À<#§ÝÿúøÀ=k-àãÛ@Ãf0‹Ž@'9¾g¯<?Þ:Gĺ¯"?æ"äÁ5>ü@	~?íëÑT›ä¿ïO±^p‡?ï·l]¡E࿺;ùÖEF†¿åèQ'¿è&ch¿ðUNASNone?îD¤·ÚÍA?»&~܇?«µ´ƒ/ö?»&~܇?Ý	Ò|96'?ÈèŠFÚÝ?á{Áãd¿?ÈèŠFÚÝ?ëÛ<¤?§ÌsJ¾±?À"ßÅoá?§ÌsJ¾±?ÔI`ô.?°Xރý|Í?åÛO…èür?°Xރý|Í?íþm[Å?¾Ð÷ T֓?³x4'.U?¾Ð÷ T֓?»\·LC5Æ?º"­[9Ùã?ì"iw™G?º"­[9Ùã?誁µf¦?³;¿à€ü?ÍUù*g¡i?³;¿à€ü?˜*ß°1ê?ƒuìèY?ï>©9¸€?ƒuìèYMIXED4FGL J1015.1-6353¿åP4†'!À.ÝÎ|Ð5À:yªÜ·ü[À<(íA°¤@z¤®Ë"ù?üü|¢èÍ´?ÓTª|?ì?Ü9ïô8@—€)†?ú}YÊ¡¤U¿Ô(ðd+£¿äõiøØÄ¿àä›ök+È¿ß,qãr*À¿ç'vµiù¿ïþÎÝHEUNASNone?ïå™Þý•±?f59Uà©ó?jf đW?f59Uà©ó?ï4S$ó^?¶£¶@'ê?™u›w:*;?¶£¶@'ê?î²bÛÂ^	?—
þÙý›?¤ÙÒFmÔm?—
þÙý›?îÙåJ9?€GóÁI?¢nA³øi?€GóÁI?'£æ'?Šo­}uMi?‰\¶uûn?Šo­}uMi?é®<|"'?ÈÉàOFËR?ÉGÒ
±ø?ÈÉàOFËR?왠4)ö?¨ºàdyê6?»2ÿö^°S?¨ºàdyê6?é2œx
?®òÚxh
ß?˓7™ŽØ?®òÚxh
ßAGN4FGL J1015.5-6030¿àÈCë^ª¨À	¾±›îÞpÀ8¼o´ëÀ;{'¾Šë@ÁIÿþR@Ž¼g#ü?¹µ¥ÿ-?ÄÂÇû¬´)@¨É¸EV?ö`õ˜ó×S¿ÁO¿Ez³z¿ã'Ž½É¿êw$>£©¾¿ëèU{\˜¿àÑÉ oâ¿è½Êeê?¤UNASNone3FGL J1016.5-6034?ïǂ?àÀ ?ðƃÑ?|>àŒ??ðƃÑ?ê=§2(?Ãj~µ"ó0?Çñc7»a?Ãj~µ"ó0?ìÓÌÞF?¨Ë˜ñÞ<&?¿ÙaŸq
Î?¨Ë˜ñÞ<&?ëf~>Ü®?¦Ò¾u¾k?Âf¨J?¦Ò¾u¾k?èõ˜#‰Y?Ç
ôê¤?Ì)ŸqÛö?Ç
ôê¤?ÌÈQ:ã´N?Îýl‹Þ3ì?èÍë±Gí?Îýl‹Þ3ì?çz¯1—â?³^€aw/?Ñ
¡œÐä<?³^€aw/?Ǩq¸â?¸Á¢]s´¿?êùã È?¸Á¢]s´¿MIXED4FGL J1016.1-4247?¥íÆrŽ¿€@&ùþɟãÀ:H¿è+ÎÀ<L 鄓x@ °æãÏGÑ?ûtyŸ(NÔ?ÂNÔ8üËÃ?Ä+S?î¦@—ԝ{¦@&ÎEÃö?æúÂG¸¦¿ê1s	â×Ñ?æ±x7I¿ÛX'}ÆV¿Ö8\½Æ¿å@W©4APUNASNone3FGL J1016.6-4244?ï÷¬3q"ã?JN+p?P§™"W™?JN+p?ïÖ;öm/?|€wÐÄB®?tâx‡ØV?|€wÐÄB®?ïåT4¬ýF?pt˜"ûå°?j«ËHú?pt˜"ûå°?ï¾å‡Èzœ?e¡ÍhÕ¶¾?€FþÃú?e¡ÍhÕ¶¾?ïÙ0O¬?j5~Žjw?sgòÒúÊ?j5~Žjw?ï±Ä'H?¦ˆ`\ó1L?ŸP	ÐÝ?¦ˆ`\ó1L?ï'o|BNb?Œ @ˆÎs«?‹d òÜ‹?Œ @ˆÎs«?ïA<7¸¬?‰[×ò8ÏÒ?—ØyYN'?‰[×ò8ÏÒAGN4FGL J1016.2-5729c?ëìõVƒÅG¿åًâvØ$À9[ãU¥NÀ:iÀ¬-@:šœxò@?ޚTª|?È<¨èA€?·6ј–?ò¸ ?¦=@í±GC¿ïø§¡o%þ?ïïNlta¿çU%`â˜ç¿æÓ{rg%©¿æÕ²^·po¿é¯?¨¢UNASNone?ë½ÜIl…?ŦJP¹Î?ÁŽÚMéÃ?ŦJP¹Î?ï­LÇâ_å?÷]¥*?"¬ÎG>Ï?÷]¥*?æð-®H×?¸4è­™ë?Ò¤£ÁnR?¸4è­™ë?ï÷À|˜"?v¼2ijlý?ŒÝj?>?v¼2ijlý?ëï'Ib?ÅٖÃÀ"‰?ÀA¶ÛÒy?ÅٖÃÀ"‰?íPXXÂÊü? ¨ÂÚt?µ}=:ŏ? ¨ÂÚt?æ̕û‡þÅ?¾êù6üÛ!?ÒfÔðv?¾êù6üÛ!?ëë&NÉ?´ðER!?ÃÜSÓfÄÛ?´ðER!8AGN4FGL J1017.4+5956?ïáM‡ó)@HQüLYÀ;¥
ÒÁÙÀ=
GR¤è'@¡Y¢<U@´'òÜ+?É -à
?˜K­A[õ?ÐG¯Áú
ó@a+´ä¤?éuv¿ê–ºö6¿Øv'•p?¿èi?Ñ&N¿î)gØVmË?éÒܱF^‰UNASNone?ïø¢GVðk?SÙˆÇ?Mvãˆñž?SÙˆÇ?ïö'?Û&?S",P&?RÚÅÖÔk?S",P&?ï'5ÿ/9m?"@ÌÉPÒ:?‹²€>€xž?"@ÌÉPÒ:?ïñfãA‹ï?FR@aõ;Q?]29:ï¢2?FR@aõ;Q?ïøHßþéç?N«-å<³?NÜa\Ì?N«-å<³?ïÙ*­ly?sÄHË÷ú?sj©:¥.*?sÄHË÷ú?åÞý¸?ŠŽ=ÕT"?ˆWz'"?ŠŽ=ÕT"?ï¿0|˔?naR0"?€3Ûïëbø?naR0"AGN4FGL J1018.1-4051¿æ"VÌё@*"4çhZÀ:¢ï	7·&À<;EM*Ë@I'VT'@E®æ1ø¡?˂ºZ•?ÍÔ`)‹i«?ÿñõ*¹çî@ØÌàBö?îH`A]ò¿ätcI{t¿ç‡§ßW"æ¿èa3¡˜¶¿êÐ0Áhë¿ïÿØÝý ÓUNASNone?ì	

•Ðó?ÓE—丧?¿·—"Qxe?ÓE—丧?ï»T(eÃ?"PmÅxŒ?*õóÉÓ)?"PmÅxŒ?ï¯-ÃÃÊ×?|XgÜCsƒ?"4Žýß>i?|XgÜCsƒ?ï°ў«?aðšþº¸?ƒü‹Ûr?aðšþº¸?ï‡P:øEï?—\CÙ"?Ž+ñ;LY?—\CÙ"?îIx±½c?° âÚ/Ø?«hv$ä)Ï?° âÚ/Ø?íÚ½x'±?¢×6¿üý?±*@GÑw?¢×6¿üý?픗Èøƕ?–¬™*ÒÊ9?³[A¹ƒ¥Ú?–¬™*ÒÊ9AGN4FGL J1018.1-2705¿Â…âÚ¢šÂ@8u#Ä*fÜÀ:hõZŠÀ<8a|ÚQ@ɓ¨=÷1@˜ºvˆó?ĪՁ&[4?Á½¿~/°È?ú¡Üär@!͕I¨À?ïý:óñÔÄ¿åvv½Ì¿çmâ0·-¿éŸÚÚ®7¿ä:ˆA'O¿ïúp &'UNASNone?ïùÖc#'?Då4•mH¸?Kঋš?Då4•mH¸?ïÞB€ƒ+?t~PZèÜ0?pÞ¿½'R?t~PZèÜ0?ïÔìė|¼?r	][V¼?u‰´A¡Ç?r	][V¼?¦½?_­"–‰:š?}!$¢R¤?_­"–‰:š?ïÝf8 áU?pÈUÔÓÃj?qLãþ­š?pÈUÔÓÃj?ïróú'×?–E˜–&'?'¡€´>9?–E˜–&'?îð'uý¡ñ?˜×D^¤‡&? öØ¡Ý®ô?˜×D^¤‡&?î hg"Ü?–8ōë?­ùy…ÖWá?–8ōëAGN4FGL J1018.2+0145¿ã°/²š@F³jçÕfÏÀ;$©Á/À<±²•"@]ï-õ±?þŸô╋î?ٔ"â-1<?ïýwå?@dÞÁÁÖÐ?úØ]å
‹Y?ëÿDïY­¿ç˜>»&²¿Ê7Üæ"¿ê'äÏ"£¿ïý!(n´?ïòH¢0AUNASNone?ïŒd"¥'—?•ŸHGPþI?Œæ÷]~'+?•ŸHGPþI?ëU©ó.
?ÁÌÎvs?©X3GÖ?ÁÌÎvs?ít@c"J?žÏËG/¢?´]ÿß¯*?žÏËG/¢?æùw<øXí?µŽª‰HA!?Ò
†N'?µŽª‰HA!?în;J6Ž?°4Ì/Ãç÷?©K[»@?°4Ì/Ãç÷?ÒDNšS+?ͬøà?æÝزÖxê?ͬøà?êÈn½¼¨V?¯ÈjuãI?ÄÞE	
^§?¯ÈjuãI?ÏÈâWoö?¼ê‰KBÉ~?è
ûj$?¼ê‰KBÉ~MIXED4FGL J1018.3-0703?ÑføÌHÝ@CÌÅûø3ƒÀ:¥·gà¹êÀ<c@ìF@@\ mf@"V^±f??Ðyu'
5ô?ǟxÖ«rà?÷‰÷/væ@­9ó–»?炙›L!A¿å)
`EË¿ß
œ¦"Sß¿ïÌdAÈø,?ãèߢ'fŸ¿ïýŒó˜épUNASNone?ïü#o¤[G?BbÙï?>ä"z]û?BbÙï?ïó¦Û¡{æ?Z£ß_J5?X²He4%?Z£ß_J5?ïµl±.5È?'D0¼wsa?'¤ÓĘ·Ñ?'D0¼wsa?ïþ^d[Á"?!Éí$Îg4?*¹OÏKa?!Éí$Îg4?ïøBòBþ?V³bÊ¥Ø#?Nô7^¯¿?V³bÊ¥Ø#?ïÅh ¹"­?‹sÝ?}K¯ªá?‹sÝ?îÿ±Tåú4?—eÞ+Cü? ê³X*»?—eÞ+Cü?ïîš/Ÿ2"?`Hž§7ùT?aeÐIpÈ?`Hž§7ùTAGN4FGL J1018.4+2210?ÜRi?@Kƒ9Ÿ]þ¹À<jQÎ_À=[Ëñr@%+¶ü?ñ¥"}c?çd#Ë·#?ã,ù'þtæ?õáÄüó0?þD!!㪊¿îëç?ï2Ôy±¿îéDg8~¿ïš|¨"2?ïÙ|s%'?À"v>öŠáUNASNone?ïýŠ…暏?@þµ!ô?3«ÑwË£?@þµ!ô?ïí3*Šÿ3?}ŸÆ0ßÇ?bÌÕd'¬ß?}ŸÆ0ßÇ?î«H[õ…d?˜®ý~Ò`?¥Kz?ËÂÃ?˜®ý~Ò`?ïûßxºÀ ?Bü¯ø…2?@'q)¼b?Bü¯ø…2?ïè
?²6?sÂ8´VÛ?gõß?sÂ8´VÛ?ï•Aub¥? ±ÒÂñ\?Š¿/°eÆ«? ±ÒÂñ\?î4w-*|ù?ŸIæη¥Í?¬¸/þt?ŸIæη¥Í?︿V9?'3>BqCÙ?Ð*gl&Ã?'3>BqCÙAGN4FGL J1019.3+5625¿Ü"HocÛ@I
¿cíÀ<©.bÀ=5óþj@!
"´ÛŒ?÷ÚWdjã¤?ÝEÈa-A'?àt†_U% @)!ÌÙb@ÊO*Š˜¿àÜäÝdʅ¿ïýE¥ü~k?ï¸7îƒ×¿ÑÏÜâ¹_¿âA¿Þ&çJ¿ï·a–5UNASNone?ïý¤~4Ž?4»{· †™?2ßìÖwÿ?4»{· †™?ïõ*—Qs?V»çý ÄL?U«óUNm?V»çý ÄL?ïŠL°Ãèß?‰°í7X?lÓÁGXe?‰°í7X?ïåúRÁîÍ?Tä!…gYÀ?j­G° ?Tä!…gYÀ?ïüÓȔƒÛ??Œ…=ì4	?9a»àë .??Œ…=ì4	?ï؉e]Á–?u3‰ùuB¾?s»M3''+?u3‰ùuB¾?ïËLD¯º÷?'ú ˆÝ\?zYÝÄOPy?'ú ˆÝ\?ïлo–?mJL
oM?wõ"—´±?mJL
oMAGN4FGL J1020.4-5314?Ζb¿@	•,ß?–À:Ž¸c­OÀ<Jr&Ü
@âhgs@½ºŠ&_?Îÿ*˜>?â_t¤íŠ²@)M<É´ê?þhà;"€«¿ïÿÞý¦ßR?ïÿÞý¦ßR¿Ú)ÜÈBy¿éˆÛÜ4I¿én"‡êD­¿ïóóí£*UNASNone?à'ä¿¡"ä?ÐN´~k?ß°6€¼ö7?ÐN´~k?ÒP†è‰?ȇa¯X®Ô?æÀW¸<‹»?ȇa¯X®Ô?æ(Ž­Wg?²ÐÕùü?Ó¯Öâ¥Q3?²ÐÕùü?Þ8>ÓØã9?±2¹æ¥?àãà–Žc?±2¹æ¥?¶ïû
Là?µóºÿ†7±?í"Yþ4?µóºÿ†7±?™<p+×·?£òŒbÅ	C?ï6pâÒ?£òŒbÅ	C?Æú¼>Š)d?²[¡óZU?êAPð]u§?²[¡óZU?ŸF!Q¨L?‹-¡)ÚÂ?ïÎõW@À?‹-¡)ÚÂMIXED4FGL J1021.8-6308¿ßW`0À}VlôÀ;+Ò/]À<'Ÿu{­ @!P-"áô§@¢>ü•u?Ä7A"Z¿³bÎ~€?óÔ*tGÐy?÷Ûb¯L´9?éJZÌÕ0I¿åÈÂ&*·¿è|"Ý¿äå¶rî4&¿ãžÅý0B? ý#à7–UNASNone?ïúñïñë?"NB>Òg?G¸9Æɜ?"NB>Òg?ï ß° ¼?"ÍqÞf>?‡þÈF¤ñ?"ÍqÞf>?ïáÖòj–!?qÓ60<N?n)
a/Ï_?qÓ60<N?ïÍ°˜Óe?eÛ2ÍÓú?y§Èãáu?eÛ2ÍÓú?ïûÙej¯?=³¡xý? ?@šio	P²?=³¡xý? ?íé"]M?À'=dv«?·x·ô¦ð?À'=dv«?ïÐYȄyÞ?}Ó; qur?wÓÓ¤æ?}Ó; qur?íEÙAéô?¨¸Ê¦Ë!?µÑ5òh-_?¨¸Ê¦Ë!AGN4FGL J1026.2-5731¿·GÇãۑt?–Òi!ŠFôÀ9éû±¼¦À;olŸe‹@Jê½£@|<âž4?Ŗ•BÇк?æ¢~ù˜@±À"š^»@qܗð÷ú¿Þž±{¸ˆ¿é֑Ýµñ¿¾Nx^
¢E¿ç±×JÕ¿í%óìÌG¿ïÿÚÁ,/´UNASNone3FGL J1026.2-5730?t¥
8øB?‰<ž˜'CÐ?ïÖµåÏ,?‰<ž˜'CÐ?¾kè9Z?µ­4Æ7/¸?ì2'øÝÕ?µ­4Æ7/¸?Ç
ÏðÝg?¬œ4µ†?ê<ŒȦ;?¬œ4µ†?ÂèûŽx ?£Í$"¢ó?ëEÁa×Ù?£Í$"¢ó?¢'Û·˜ª?Äø¿Cø'o?îݏD†u?Äø¿Cø'o?…­$<â?†°RR91?ï«åJhÌ?†°RR91?³ÈªÜÀ"?§"vnìÿ?íÆêé ?§"vnìÿ?s"w%ÜI¡?d^Sw=OŸ?ïØÙ¡	?d^Sw=OŸPSR4FGL J1027.4-6324?Å	3O¸¤øÀ'…‹Å›€À;¬7æ÷~À<š¿£ï]ñ@$»D;Îã?öœY~÷W?Ñ^˜¼¤áv?§C.d'®?Ó5ëŸJÞv@Ta#0†±¿ï†'_8u?äv†ºŸ¤¿ìÏ¡}éÑ?Ûq¸ß¯þ`¿á^@'—FÙ?›"£Q
AUNASNone?ïÿ:Á®î?6ÖÎVX\þ?§ÉDuƒ»?6ÖÎVX\þ?ïîF ?o.‹Ã*'?ar¹ò.Ð?o.‹Ã*'?ïà½þäÞ"?t¹uÙÁí?oBAf5?t¹uÙÁí?ïýÙ9—¦O?'°‹â/›?163'P¥*?'°‹â/›?ïÿ9d•<?T-Ÿ?f ?ßÐu͑ª?T-Ÿ?f ?ï"Qhòe? ¤ª'0?‹+½ö¸? ¤ª'0?ïȈþIz%?"E]¨·Ï§?{»€ÊÄ͎?"E]¨·Ï§?ïöŒ³FÜ?Rï1«
ªL?Ræ˜øJY4?Rï1«
ªLAGN4FGL J1028.1-3550¿íLÉ*gø@2‰)ˆ†À;;$ŲÀ<qÀã/@àåK@ðO‹XŽ?ÀŒDœg)Z¿²ˆLj;Ýý?õ$#–=â@t#I†0Ü?ïÿ¯þ_ìпïmªÈ–g?Ò×#gäè¿îx™¿YFÃ?Ò£ƒþ&â¿ÀU\ã°¿UNASNone?ïü±t'à?Rµي$?;'tÇ)Šö?Rµي$?ïé§×}ˆu?j
Ïý±Ù›?fX(¾ð« ?j
Ïý±Ù›?ïsŸÔ
¨?¦jÝÇ?'Œ}œú?¦jÝÇ?ïü˜/>åw?0ܛÛ>Þ?;>†ªu?0ܛÛ>Þ?ïó¨c‹ë†?ZzËqY¾Ë?X¯9=_CI?ZzËqY¾Ë?ïysÍÅ?šþ"Cp?Ñœ;ö«a?šþ"Cp?ï[|]H°s?'úxŸ?"tSzU¦?'úxŸ?ï×¾ P"?r«²4íàÕ?t ïØû7N?r«²4íàÕAGN4FGL J1028.4-1539¿Ú=ë?­·@Au~ºñ6À;úÀoÇÀ<vc¹ã»ý@ˆ<[Ðá/@À_@˜?ÎYßð@¿¨0ïáú±b?èu ޜØé@'
_Ä¿è!¡ÇåÝ¿ÎôK@ññ¿ì(Àéi¼¿"¿¹úô9¿çoP…S'x¿ÝݖH¬AUNASNone?ïÞÅAVü*?ªñ¢³?p_nžòá?ªñ¢³?ïôþêèR?X~3Í,Y?WÌŠdk'?X~3Í,Y?ïáØ$U?v'æ@ÎÄ?nç(djŠ?v'æ@ÎÄ?ïûÓ|ƒ"#?+(w(SN?@²
.§oñ?+(w(SN?ïõ­/èB?TjU³Œœ?T¥¢iájö?TjU³Œœ?ï͑Z}Ft?¥*ù~2Â?y7R¤€?¥*ù~2Â?ïÕV`ß¾Â?~
'‰Æê?uTÏ¢?~
'‰Æê?ïÝ~WÁ)x?eæJ‹<?q@Ô*jû?eæJ‹<AGN4FGL J1029.4-0828¿êyßofÀ(@D@ۜsh­À;!KeY -À<ŽL%r€P@6;ƒd@á#=ò©Ö?¿Ïq—ÇÝO¿·Ž†@ ?õ»‡*+M@ÅCýÛ¸x¿ì!E_…¡•¿ã2¸ÿ»a•¿âc×dÖC¿á@÷A¿á¿¾¥пÄO1ÁnìUNASNone?ïýóW>ïï?!ù­…ËÝå?0eFš¼¶´?!ù­…ËÝå?ïóa?Y8žŠ¢¹\?Y=Ô'I?Y8žŠ¢¹\?ï÷DõIåõ?YalŽ—°?Qvþ@—ˆ?YalŽ—°?ïúǦ"¡/?0ü2Ñâä?Dáe8îìE?0ü2Ñâä?ïûadÞ¤?:ÑIê,‡A?Bzp%d?:ÑIê,‡A?ïÄ;j~î?Š–´¨aà$?}âJ¯ÈýW?Š–´¨aà$?ïöbO€pÔ?g›=è~¾&?S;aF–8M?g›=è~¾&?ïʒÄ×ú—?pãÅÛÔþ?z¶¶^Ì>?pãÅÛÔþAGN4FGL J1029.9+7335¿ïŠ4ûpŠh@Cü¥aMø±À;–|tÅ¥À<ö)¢¹ @ §N}ça?úÌ
Jݐ?ß.M»tµµ?Õÿ™¾, ó?üLØç&?ûÏ?Ž
oE?ïû³ûð¿ì\šP}F¿áÃ9¦û¿µ;—Ÿˆ4Ü¿á"ÀĀοïÿÂÃ^UNASNone?ïôá°M~þ?J÷æ™t½Ì?V<ŸmA©?J÷æ™t½Ì?ïØӆ$qÏ?y0¡Ò²ó½?s–=Tü>?y0¡Ò²ó½?ï·g'áC§?zæHðµc?'&E÷H0?zæHðµc?ï"ë]lÔ?r&š^;¥Ã?ŽþÅ/"?r&š^;¥Ã?ïô§Å	?YÂߪ®?Wа½e¼H?YÂߪ®?ïN
«¨ÿ'??†OPOm?–>J'¿G¹??†OPOm?ï´nÊÁ\?ƒ`=6%-Ç?'äM?v
?ƒ`=6%-Ç?í¯½qÝ_d? ÞPb+æ?²'r^ßb? ÞPb+æAGN4FGL J1030.7+6118¿ïù¨.v¤¼@HBã¼ÓZ†À:pöa7À;ÐÑPÀô@>/»"zù@™……žÙ?Âc'¦b*¿¦¿$ÝHß²?çgºú<q @ÐË}í@¶?ïðL2Þ¿èò‰?.i¿éüp>–©¿×ÿÞ<`Ù_¿ïÿþªJl¿ß&|¡;N‹UNASNone?ïðf(M1?`¨ü08<=?_3¯Å)G?`¨ü08<=?ïñC'Y'õ?^[±¶3?]xÛsWµN?^[±¶3?ï êÏIÝL?†|E É
Ð?‡ÅLÊ<þ?†|E É
Ð?ïגÁ–ÁV?[-,îQ€?t6Ÿ3?}-?[-,îQ€?ﷂÅœç?‡¨9¶°?'N¶±¬Z?‡¨9¶°?ïÆ@dQÂ?}Bï±°¿	?|ý_À¯/?}Bï±°¿	?îÝXhKîÁ?™V¹®å~?¢*ywÑwö?™V¹®å~?î{_TN`á?•àЫLÌ?¨J
½­¦ë?•àЫLÌAGN4FGL J1032.0+5725?žòuÄ@I"~bÜn+À;<Uw*ÙÈÀ<†±	¢@@(²-9I"@ü¦y{ìà?ÐPP~?ª÷J=ªŸ??ÜÞÔa@·«?쥗•C¯¾¿åŸRu¿é|CG}m¿ã à_Ñ¡É¿å18‡0
Š¿ïù
By!T¿ÔcÃHê€UNASNone?ï÷®6Ñ?TûYd	¾¿?Q£rò?TûYd	¾¿?ï6Æ]xÐ?Ÿ{˜Þ¥ë¡?™'4Xi|?Ÿ{˜Þ¥ë¡?ï{Øó™Í?ˆeÍn›.¾?"á‰nêt?ˆeÍn›.¾?îÒK¥"—b?ŠŽ‰	o¢?¢ÛE¯ŽWÚ?ŠŽ‰	o¢?ïùŠÓ‹¶?Qˆ€Ÿ|"?K'ÕÄ%(8?Qˆ€Ÿ|"?èf#ë¾?˒e¬ÆáÀ?Îgs»¨Q?˒e¬ÆáÀ?ï€fG1ÂÆ?Œ$ª‹,º
?æn)@z ?Œ$ª‹,º
?ä€Þ¨¨'j?»ÚâlÏ¿¤?ÖþB®®Ý+?»ÚâlÏ¿¤AGN4FGL J1036.3-5833e¿ïcˆ'Ø'¿Ç;»cÀ5õÆâ¨eÀ9~ƒujæ(@ ï'v"ò?þAZ=c8?"+¹äŠ%*?¢˜ÕÏTçc@ü†~3â†@H¦³2œà¿é\P˜žÇ×?ڮפJD¿Ü
Æ(Ä¿Úª¨ À€¿ãʍÜÕ¿Ø\$"ô÷ŽUNASNone2FGL J1036.4-5828c?é̎‹‰ó?Î'Ź)¤?ÈÍÅÁÑØ6?Î'Ź)¤?ï¹\e.?"·fšO`?¨æ•U$:?"·fšO`?ç"]óÙµ?³yªê¦†Ð?ÑøÙDL—?³yªê¦†Ð?ïzïƒ?ˆÀŽ~œK?¢/'1?ˆÀŽ~œK?ïëÂl‡Ï?¦fÊò#•Ô?œ¢‡»?¦fÊò#•Ô?î7ô‰»fY?·ŒÐr† ½?¬€·dIšm?·ŒÐr† ½?ëŸIìTžà?°Aµ'y,?Á'ØN­"?°Aµ'y,?î:b† Ú°?©ÿ*Ò©•?¬Yסaðþ?©ÿ*Ò©•AGN4FGL J1036.5-1809?ë6*üOhÀ@AÃ\á'À:Ž%ߍ™±À<^E¾P2G@^û+9À@P1ônÒ?ÂäºiÈƃ?¬Bþ'Q?æMΊ<."@<>5šÁ¿Ó¢<UpË¿å««Ÿ«y¿êJ0'|G¿æÝ´"9¼¿î~"_¦XÅ¿ïìt½—$ÊUNASNone?ïö5)56 ?P ›myÞ?S•­ßËNí?P ›myÞ?ïï™Ãh©?eóÚ.ìpç?`ìfYtD?eóÚ.ìpç?ïÛqä&Ž=?pàtµc?rG
Ï,=Ã?pàtµc?ïéK
™?PYh/‡?f´òÐi|Ø?PYh/‡?ïæèîQ½ô?d÷bq'§?iÂß³æ?d÷bq'§?ï½àÏî|?‹_IÝ0ו?€‡ýÎÄ?‹_IÝ0ו?ïÇ¡jδ?€žy;£ï²?|/uÒ'Ê0?€žy;£ï²?ïTÑ"ÇÖ?ƒ9"1GŽ?•eÛ¨½
þ?ƒ9"1GŽAGN4FGL J1036.6-4349¿ä
HÙÙó@):ïÔ8ÑÙÀ:Q-ÛÛ]‰À<Ab8Ú<!@­'¦Û÷b@CptÙÇ?À2­Ò5ÂZ?˗ä£-A,@	,辚Úâ?ý=e?tà¿Àõ5v¯_¿Þi%}½ðç¿ÛK-zâtT¿ã?Âùt7¿è¥¶ÞMþ'¿ðUNASNone3FGL J1036.4-4348?í‰5dՆt?µƒƒ'Á?³¶TØåØä?µƒƒ'Á?íº?Ï×Kß?±sc¢WQw?².³"…?±sc¢WQw?ÙWõŠ?š$¬3"y½?¥çrk\ŽY?š$¬3"y½?î¤{†NÓ?Â‰	+]?¥¸Nö¿+Ó?Â‰	+]?ã»ãÕõ6ñ?Ë´C}‹Ð?؈8T'?Ë´C}‹Ð?à%×½Á—?И‰›?ß´P"|Ñã?И‰›?æغ–¿J?¿Q"ïô?ÓúNŠÒm?¿Q"ïô?æààÔÛRæ?­«©ƒÊå?Ò>>VIZ3?­«©ƒÊåAGN4FGL J1037.8-5810c¿ïK4\\?Ï7äGè¡êÀ8¹Š>²Ã6À:_SUªL@±Ìp±m÷@z…\ '?ÁBL€·'?Òã%Ô¥ß@=B€®?ùÝ(¼Ü¿äÇÍ¿;Ò¿Û*«º®g1¿çƒhÀ2à}¿èeÌþJô¿ï›^?ÑQ¿ï¼~Æ.£UNASNone3FGL J1039.1-5809?ۘ<–r?Ô&ï+ÔD?â3áü´Æò?Ô&ï+ÔD?ÊAT‰D?Ãùiì`o?éyoªÝ¹¯?Ãùiì`o?ÜÖÊÍL'?¶2f[Ëû
?ᔚ™sÙì?¶2f[Ëû
?×'ÿÇK?²ö@¹¦T?ä|7Z?²ö@¹¦T?³gÉ-ê?µ"Ævëp†?í"ڇ?µ"Ævëp†?‹rwÑ#ÇÑ?…e£¹Q?ï'6 ÖíÁ?…e£¹Q?º¿'÷tý>?ªÊ;SçSy?ì¨
Á`X?ªÊ;SçSy?"H㳖z?wi'%"?ï®Üpü
ú?wi'%"4PSR4FGL J1039.2+3258?žƒ51Ã¥@Nvߤ?åÉÀ:¯û–ä³sÀ<©J–ý'@ҏ7@.@ŽIW?ÀT;ª·#?³Ryt‹K?ð4äù}@³¨Ž?ïÃùߪu	¿ÏZ|ù$ïy¿èL%r€P¿åOàèãƒÈ¿ç|ô¢©¸¡¿ïÿ€H»ÊUNASNone?ïùÕOc{·?@'zoi9?HªÂééëh?@'zoi9?ïèz4Eú-?h¤­£V¦¿?g…ËŽ
ә?h¤­£V¦¿?ïÉÝ-ºoÊ?w"»A]»?{iDtF¡?w"»A]»?Ó+¥?n/ü	äÏà?‡ß\Ž¤²¢?n/ü	äÏà?ïí½mçÂ¥?`*.º¸®?bB'^#?`*.º¸®?柳o¼Æ?ˆÌùÞÌÖ<?†¤®:©?ˆÌùÞÌÖ<?ï|•è½¡¿?ŠÇuGû?mBæ"ú?ŠÇuGû?íè°«âz?˜VPÆKfK?°ºz¡Èy?˜VPÆKfKAGN4FGL J1043.0+5316?ç!< ÿ@K[è>BZîÀ:ØâäfF†À<¶˜x1j@Ā=¨;@ˆœT?ÃO ;Ê0?Žü>:´m?Äàw9@@œ¶"‹ë¿¶ôŒÚC'â¿ãÝDÿŽk¿í2¬'ª¿ÚiVpOu¿íO|	eÚO?ÓH>Þ:KUNASNone?ïåÐúX÷?tïö)5±?jú/
æâ?tïö)5±?ïö"8g¶¯?R¦]cÃi?RَñYÒå?R¦]cÃi?ïÃÅÛ§¾?~"R8°?~SÏhé?~"R8°?ï÷>ª#™Q??}3ðçñ?Q'«PY>u??}3ðçñ?ïäãÅ˜?pÏÇägÁƒ?k~<N@|?pÏÇägÁƒ?ïÖ+Êw÷¢?w«Âh~DX?tê˓Râ?w«Âh~DX?ïÄȉœ ˆ?õ[ˆ,+?}›»"ÑtP?õ[ˆ,+?ï®Õ'[°ø?xº^?"J¶*ˏô?xº^AGN4FGL J1044.5-1439?Ô˜ýù{¾@C©~+VÀ:ãwúã`À<uMËdíÀ@qÃ/?¨@CQÞïå?ϵ»£¯?¿3çmår?ðŽ†@ €?ú¶Qô¿äß,D+©¿æg öo³¿Öe:´e¿é
¸UFƒr¿åà#¡oÑÊ¿ïäê›íUNASNone?ïüsD´ÿ•?5µú¡û†9?<eÚøŠ­?5µú¡û†9?ï×ÍʁK£?}Hb+§J?tµZ¿?}Hb+§J?ïÏ6Ç<j?vF³ [ó¤?xdœgúB*?vF³ [ó¤?ïº/·äÄv?d—nº©yØ?t÷Œj?d—nº©yØ?ïôà\v£u?R.Ï]59B?V?GD3tð?R.Ï]59B?ï7ÊîÀz?  ‡¿»?™¢0–ö§?  ‡¿»?ï|Æ
w
?š]+,¾?g>±N'?š]+,¾?íà6¬9"[?›ç2Þâi?°þJŸ}·¥?›ç2ÞâiAGN4FGL J1046.7-6010?༩Ž%¿z¿îócښë©À8"k·ÞþþÀ:lµ…ˆj@9Œ‹"Y@ÕC/Ш?½Ï€±@TY?Øm©PÆÂ@ܚ )֓@MNB«Ì¿ã:©´™Ð ¿Äo-ŸËaé¿âÍQ¢4è¿ê_Á†"¿íA(¿<¿ïÿÿÊPËUNASNone3FGL J1047.3-6005?™ê£kbK:?«}Ë\CÏ?ï0ªä‰pÆ?«}Ë\CÏ?À<¨‡ž†?·a§Øõí?ëðÕÞyž?·a§Øõí?žU‹Lϼ?°·cÏ K?ëXj,Ì?°·cÏ K?Ò¦z&Y(?³tãîܪ?æ¬òBìÓl?³tãîܪ?¢¼eOÔÃU?ÆG'Ù¿'?îÔ9«Gkú?ÆG'Ù¿'?…zÿ0¿hö?†ÚE½@Á%?ïªJÀÌ?†ÚE½@Á%?Œ=N¥uy?',ŽœBá?ï
'nj*?',ŽœBá?y0/AéÞÆ?l Ò³†?ï͟¡«¢?l Ò³†PSR4FGL J1047.2+6740?ä46+Ç?U@F­…ƒb°À;xTFŸÀ=å‡ó@ y¨ä^˜?ü'Dc_–?ÉXOwa‹`?¸.çI$â
?ðêÜ0@	LG²òA¿í$¼B;
ó¿áÁƒ(yF¿Þ€žÐe3¿â@¬ÞDïH?˜·G.%5¿êq=Å]lÃUNASNone?ïÿž3À2>ü`ò!4?{«gMK•>ü`ò!4?ï÷Ú+§p?QS³¹ ?PK¨Ê°$Z?QS³¹ ?ïò¡èȀã?p{·2c?Z¼.cÿz'?p{·2c?ïÿS"ù?ÆøM+G?'Û#Ò?ÆøM+G?ïÿËh¯Ó?îÆ@f?š~Á_?îÆ@f?ïÝ›Hà?rcP¶•?q{²iþX,?rcP¶•?ïôóò‡$?nèõ_?Vxg+?nèõ_?ïýq$&ó+?/@A»l?4vݧ:º/?/@A»lAGN4FGL J1048.4-5030?àe¢ïX½Ü@èϦ›áÀ;~‡Å[¿À<€"Œê^®@"ží'`A3?÷&Lëk…?Ùޘ§+R"?Ò¹Ù« ê@•‰ïØj@@7Ӏñ¿Ó@LyË¿ài}Èâ¿ä§ü~Y®¿äHxÌE¿èè\૦â¿éMŠ'$‡õUNASNone?ïò¢žë?TÇd[àÙ?[Ãâì<Še?TÇd[àÙ?/6Nq?–0À`Y'T?‰™ô$­óé?–0À`Y'T?ï™^ôŠ´'?'Lÿ¿=Å?‰¨Bî€ëg?'Lÿ¿=Å?ï}ίÐè?z¶§•ßfŠ?F*Â%í?z¶§•ßfŠ?ïØIh\hi?pŒñâÓ@Ò?sÛK°Ï‹"?pŒñâÓ@Ò?íÙE£ù?¶"ñŽcŠ³?±5ÒÞiÒ?¶"ñŽcŠ³?î"Gîší?šUþfoB?¦¾[…aÔ0?šUþfoB?íh›Uo?¦"¢–hBÒ?´»%S£J…?¦"¢–hBÒAGN4FGL J1048.5-5923?ØÚç¡S;*¿ÅU€e-À8µýawÀ:Œd×-©@Ì22Yò@9fâ?¿äð/'ŠÞ?à€`b–M4@èîkƒÙ?øœ¤Z诿ݫ^ʐ²¿áa%Ie¤ ¿×ÐfíÖÞ¿êS恩¸Ì¿ïÿÞý¦ßR?ïùT_}¾óUNASNone?‡©£¡)Î?š¹˜VgYš?ï¡Yq`jy?š¹˜VgYš?µ'k›?¯L?Iœ>?íMßoÍÔp?¯L?Iœ>?½ŒðÎ^È?¨AÔ	!ÔË?ìNnæ4'?¨AÔ	!ÔË?­W­©?Ûì&8·?î.J'í¥?Ûì&8·?i§âHU'?£†øFí&?ïæXÅ°?£†øFí&?ŽX»Ž°?'pVNs/?ï¹ÆœÿL?'pVNs/?£‰y·0¼?š–ð"æ€?îÇhdËå$?š–ð"æ€?6ÃÀìؕý?3}ZžÕ6'?ïý'‡û®Ú?3}ZžÕ6'PSR4FGL J1049.8+2741¿ì݈À>°%@O‰\Rç-¡À;$jÈ˶LÀ<ÂÉø6{@Èey+ü@c'†Wv?Á?wd:'"¿ª†»›w_?ê_
Awn¡@Qu=™¿?ï¤nß±¬¿é£=òÔÉ¿át€Û\²ˆ¿ÞCO
)N®¿èê¢5Ié?i…ÖüíUNASNone?ïú=Þ)bò?@¶J°tL?G‡*Q	?@¶J°tL?ïõ˜H²?T¬ÎoÜ&G?TÏÝèÆÚó?T¬ÎoÜ&G?ïìJ•iM?b´']ar?cµjˆô€§?b´']ar?ïðM¨qµ?B´-Œ-?_eôãV¥ù?B´-Œ-?ïëµ-§`µ?]¾>†!é?dJҚ—Êz?]¾>†!é?ïÕÔ}›6R?x!ðJcS?uÁ1´ë?x!ðJcS?ïÔT]¥L«?|ÏÉeëël?uÕÑkî‡?|ÏÉeëël?ﰒá]l\?oïOÝóB?ƒÛG˜&É4?oïOÝóBAGN4FGL J1049.9-3658?àùØþ@3ÒóÂÚۃÀ;o…j7¬?À<½¯€‹¬@ü<'UÓ?þ#Ÿý`éO?×îS/Qý?Õ<캨ÝÚ?þs™õßëŽ@nÏ[rl"¿Îˆ""ꐭ¿ì6J	8æ?áO܁u¶f¿âÉ­"K¡¿¿Úû¯cZm_¿ïý_ ÷ÇLUNASNone?ïù~@Í¥?BÍmr˜?JýU
U?BÍmr˜?ï鏬—?gß—2˜?fpSRùÿ5?gß—2˜?ï¾Ò€ÀÚ¦?vŒ€Ò†t?€K_Ӑèp?vŒ€Ò†t?ïén
Áà?NQ`¾c1Ã?f'ÿÖÁ@?NQ`¾c1Ã?ïùÔä!«?H°³ª†à?H¬m©c›?H°³ª†à?ï–gû¼ÏT?"@"š±Yš?ŠfŠšþ?"@"š±Yš?ïšì‹e"?‰‡‡ß
?‰Dùh+L?‰‡‡ß
?ï¦À'³¤»?x³kÊÏפ?†OÛ¤DÝ?x³kÊÏפAGN4FGL J1054.0-5938?ìøFŸezG¿´ê}6âjÀ:*&¨«À;zKìgœÇ@¥ðj
à¯@DÍ$
¡D?Ò=Äòø6?ÛFuš¶Ð@	Ž"ü¡¦®?ÿ[Fo¦/¿â¿°"—ª¿ààŠï²ªã¿ã ¢Bµ‡¿àýT‰Å@¿ì¯¹"<¿ðUNASNone?ì¿p?³Éã³J?º‡"gP?³Éã³J?ë…B×bta?»RØF#?Áêô¢v.}?»RØF#?ëM·ò†V?§:I"˜?ÂÉ 5æ§û?§:I"˜?í8?"ä™mM?³÷<ӆU?"ä™mM?æ` ó?Ä:HüG?Ó?ãÔ¿ú?Ä:HüG?Ò{ç"2Þ`?ÎSï€ù1?æÂ6fÐ?ÎSï€ù1?ße¯liµ¦?¹"'ˆÜœž?àM(IË%-?¹"'ˆÜœž?ÛôhݏÖ?º˜#«^p¬?âˑ8w?º˜#«^p¬MIXED4FGL J1054.7-6008c?ï«D«-–¿ßt_ƒVRÀ9>¡ò-¯fÀ:ºôƒÊû;@ ¬ÿ"Ë(³@#éÁЈ?Åß¼™Ï?´}áWHfK?ôc@\¢@x•±'™¿é–:‰hÊ?î6êx´G¿ëB‹`òË¿á…!ýÖ¯û¿äw'¯c¿éÎf*…UNASNone3FGL J1054.7-6006?ïÍíÔâÎt?€~Z"´(?y	"h9¿?€~Z"´(?|11"?c¹ìS?‡ þrù?c¹ìS?ìçÊùt1?ª?òµrî?¸ÇY©ì,v?ª?òµrî?3´@?xd›ÈŒc?Ž–³¡&e?xd›ÈŒc?íöaq<¶È?´ÅœqO?°Lôx@;?´ÅœqO?íLæ6™f?Á2"æ?µ˜ÎPWË?Á2"æ?êìx—Ò€Q?´¦~:Û?ÄN µþ»?´¦~:Û?ëeä
¹¯—?³'º'µ?ÂhoÉA£?³'º'µ4AGN4FGL J1055.6-0719¿Ú'IÚI?@FË  ôØÀ:Òs«ÉGÀ<}4#;z@öõtŒ?úfÉèì¾?呈pSO?ãè›)¼'ì?ýR0",J@"B)›.ð?ï¸;Ÿé?¿á jÓ¿Þ*¤ ¿í·¬ª–¿ïêԟ©þí¿ïýÁÆßMUNASNone?ïéÌË'ä©?'ɹ:ªf?f34"ÂÿH?'ɹ:ªf?ï¦ñ…W²?"	ûq;?†Cž¦£â+?"	ûq;?î><h͎?—geî0?¬7*O$?—geî0?îôW'¯Œ?ˆvAm/Ú? º"2`B?ˆvAm/Ú?ï™
K™—§?Ó¹ϲ£?‰½m#èê?Ó¹ϲ£?î˜U}Ϩc?±é'γ¨?¦z¨•ÝÒ?±é'γ¨?ìá°™Ãê?£»'j±'L?¸÷Z{ŸÔ3?£»'j±'L?í@€‰ÖÐ?¦8…g?µûÿDû#ü?¦8…gAGN4FGL J1055.7+1033?ïߘýp^@M¶0©8À;mv"Û·À<·þ^?Px@L)ÿ'׋@Õ`EK?Îú0³&2š?Šæ
²ûj?¸åõåZ¸@xއ_ZY?ë;>À<{¿ê©p§2'?²zò9˜Ó¿áöRš™Ê¿àsø^K¿ï—m¿öûuUNASNone?ïþܧ¾Óî?úN"Ä?"5-®÷Ò?úN"Ä?ïöI{Dø?Uß7c¾ž:?SmÔö8?Z?Uß7c¾ž:?ïõkuÄÓ?]¸xµÓöà?UÅ(Ò}Ùÿ?]¸xµÓöà?ïûio|±ú?)ùòH×?BZB®Øë–?)ùòH×?ïÿ/Äyþ/?w½CÔê¼?qÅý8?w½CÔê¼?ïÔ³
>W?"OZï?u¦wޓà¦?"OZï?ïöÙ¬··?g£ñЪ	?SúMÄa8?g£ñЪ	?ïó¿'GŒ?HÀ‰²0Â?X±R>W|?HÀ‰²0ÂAGN4FGL J1055.7-1807¿äs*D!B@Bb¢"ÕÀ;†PÎN­À<¦üZYê@`àëgÃ@T"\Böö?Å
{"Üß¿·Y ¾Í–Ý?óUE¬²{@'óÒö­?ï'S‰êÏí¿ìîbHŸ¿áé€C‡>¿ã")Zl] ¿ÏfD˜
xT¿Í^;I­UNASNone?ïûΩ,ö?4(=!ƒ?@Å[€…ÌØ?4(=!ƒ?ïðN/2s?`PвG€ì?_bá†:ô?`PвG€ì?ïäÒ=,¹Ð?tZF¥fã?k-Ãþ_¨?tZF¥fã?ïúˆ>ÓOs?5Nv?Eßt¢Þˆ?5Nv?ïõ.VeÎw?NU{X ?U£SZQ;?NU{X ?ïºBgóH%?‹Ý Ñ鎜?ofD\?‹Ý Ñ鎜?ïÛäÐ(Í?}í{R"É?r
ü¸7íj?}í{R"É?ï½¢Qq•?x$rÚùÅ?€—aTÆ»?x$rÚùÅAGN4FGL J1057.6-4051¿×÷ZP@1«\9¼ºÀ;T'ÏR¹
À<¯ík¨Å‡@!Å.	¹?÷ÏY­€?ÕÛt/|ÅM?×­ãænß@®¤Ã™Gd@ЈÐº%¿ïÿóÀ¬ƒ?ïÿÿ&¦³?Üe·>ñŠ?œÖƒb~-
¿Þqá">éu¿ãJ½Y<\UNASNone3FGL J1057.6-4051?ïýӒ¹«ˆ?4:Í,~?1ck˨r6?4:Í,~?ïç4¹^õž?nü"†¤eK?hËF~®Jš?nü"†¤eK?ïX¸Jߢ=?'ɐ®î¨Z?"èö,€y?'ɐ®î¨Z?ï햾?b¹?M—Å—d.x?biAÏ»?M—Å—d.x?ïþO´Sx?) ‰éžwÎ?+½ÝÑ@ø?) ‰éžwÎ?ï|ÑùB²¾?™Ý7!VS?eÀÐÊpB?™Ý7!VS?ïª523P\?‰¶üƒá?…r³s+é	?‰¶üƒá?ïԌ[ë?i–~À{ù?u¹ÒS‡W?i–~À{ùAGN4FGL J1058.4-6625¿ïQØMŖßÀú†×6&À:©ˆúååÀ<@—ŸÄV@ –|¨È?þÄâ½ÏÙÈ?Â%;8eL5?µ¦?piu?öóFc'ŸÐ@à¦ÉWø:¿ä|Wisa?ïò±}»í¿æŒ"ÎX¾¿Ò¤e¥vF®¿æ,SzÑWv¿ÙÞ¾‰¾UNASNone2FGL J1058.7-6621?ïü>D^SÈ?3Õ7Þâƒ?>
Þ
Dü?3Õ7Þâƒ?ï⋶.S?uø,N9Ó?mtIÆxÿ?uø,N9Ó?ï܌±ºÞÊ?{Y»ºš?q¹§3¾¦ø?{Y»ºš?ïÐ	œz¹H?_ÂEÚÓ<?wû1á×˜?_ÂEÚÓ<?ï÷­C°*?HnT+6%'?P¥z'UZÙ?HnT+6%'?ïB1"]Ö±?§ý`'Ÿµ?—¹Íyl"×?§ý`'Ÿµ?ïª0q¦¥5?‹9gd†ó?…s㈘Bì?‹9gd†ó?ï5¾¨Çµ?Œu×6vù?œùH0s]?Œu×6vùAGN4FGL J1058.9-6101?èZh'º¿ñ"ӟNå@À9¢G«<#À;$•%–'~@…¿9fS@÷xmži?Êðmü1ê3?ԘL½rç©@™È î!±?÷ê–߀Å¿ïÿ¸8º1?ïøVˆ¢ÑQ¿à2Û>Õ}Ë¿ã<æp–¿ï—_'œ}?жƒ_E‹UNASNone3FGL J1058.5-6106c?ë´:¿bM?ÀyƒéGñu?Á/½vÊ?ÀyƒéGñu?âÔ"vÍfÑ?Ì%;¨™š?ÚW»e2_?Ì%;¨™š?è+5X¯ø?®êX¦nÆ?ÏS*@Þ?®êX¦nÆ?æ‰CøÂ
?±¾BÖ2^ô?ÒíÕx{æ?±¾BÖ2^ô?ÝRe9âò ?Ë !äè]³?áVÍc†ð?Ë !äè]³?¶iÈÙÖ©"?¿'0ö†ÉL?í2Æå	ã?¿'0ö†ÉL?Õ®ŸÓÍû?¹ÞK
¦ˆQ?å(°A?¹ÞK
¦ˆQ?¸Ûãëø6?§|¾³Øª¿?ìü¤ƒ'€ù?§|¾³Øª¿MIXED4FGL J1059.4+2148?Í!ñ;ý…@P,{‰
ZÀ;N1‰åÇpÀ<•ÀY÷Ã@ddàÕBg@îà¹Ü?З¶€G7?¹d
ý´÷?èñ'?_‡?ìKV^~ª¿Òn¡¾/•¿ã­`öºÝ¿âл¿^OA¿éšº–icq¿Ê÷‡‹z¿ïñd "‰UNASNone?ïÔ±åƈ?°'=¸km—?u§{­iÿ?°'=¸km—?ïoÔj6:á?˜žåàydá?'r°¡õ?˜žåàydá?ï¨\=v5Å?†%•™bo¿?…èð©Qƽ?†%•™bo¿??Öå?uŸdv܇(?Š°ËÖË?uŸdv܇(?ïôÿž†=q?\òQò¶?VÂöDÍ]?\òQò¶?ê‹1¿j¹‡?Ƶ|	w?ÅÓ9Uã?Ƶ|	w?ïŽtÝÁ‰?‹´gmzìU?ŒbýÁ°eÃ?‹´gmzìU?êŽÝ?µ†Á;'T?ÄE¥ùĎ?µ†Á;'TAGN4FGL J1059.4+0226?ë]R	HdY@JɏÙý7À9ÞkÑà2À;òhÒQq@‡séèw@½‡Ý¯s ?ÄåýJn
O?Á9ul"§?öÿ\‰ÉB@I¡yŒÞË?ïÎ` ©®¿ßè©¢%YV¿ßÙ=ˆ÷Šæ¿ãX{Â=ä¿ë²‰ŠWÝ7¿ÞAÜCbU`UNASNone3FGL J1059.3+0224?ïöﱺ]ñ?Oøgcž+k?R œƒý?Oøgcž+k?ïð)º¨KÓ?^uáì·(l?_¬ŠO3JÙ?^uáì·(l?ï6¼ÙÞ?'¦íx<G?™(|dÄ>£?'¦íx<G?ïÆ®P=³?bñ˜Dk%#?|¨×ùFj'?bñ˜Dk%#?ïµ"Ì'z?ƒV‡I؊Ÿ?'¸šÝËw?ƒV‡I؊Ÿ?ïÂ"€J?Š'5"Aa?~îô½Fà?Š'5"Aa?îËí"'l?›€õ¬ø™?£A'º›ü?›€õ¬ø™?ï$‡(A¬?ƒŠœR
ð?›ïÐ`{?ƒŠœR
ðAGN4FGL J1100.0-2044?ëù£æµ½M@A‡´€¥¬ÍÀ:ÁçIOÕ*À<"÷z€Ï@@¸žÂx`@SÕ4z[?ÆÆl ¾4?¼C"Ó†û1?ñu~æ­?÷µ×8XŒ¿Õé4 G3¿ãgšx
ÿ¿Ùsÿ*¿åÑG@~š¿ãæàtI~¿é¼«aÃ'UNASNone3FGL J1100.2-2044?ïúd¯åÙ??¦ˆ=J"?Fo"/ºÑò??¦ˆ=J"?ïÐVw0
9?€÷Ž.é?wÔÄ\J·"?€÷Ž.é?ïÜ£hº?rqM°·?qû®UùÕ?rqM°·?籠S-ÆÚ?i7½¾2qj?†žëBL¹i?i7½¾2qj?ïõ4ê]V?NaÊØ_õg?U–,BüC{?NaÊØ_õg?ïti'0?¥T‡(Ä=‰?ŸqrÖX´?¥T‡(Ä=‰?ïћª¯°K?|MŒÂôñT?w2*À5L?|MŒÂôñT?햤Ÿå–¦?œWPN"?³JÛÓJÑ?œWPN"AGN4FGL J1102.3+6715?íÙ/<Q @GJ²BÀ;è¤nòÀ=0fC*÷û@!PØ?ɵ?ûV³»ƒÏ-?ÏAÖçØÂ?¶î•ÊW&­?êö5çB™Ù@ÓLÙ!™Ù¿ï¥íÀ7h!¿Ô°oó ?ïù0¾
í)¿æ{›¢|K?¸Ï2ؚ`¿é8%@+i:UNASNone?ïÿiDð¨}?LbÑ?×^Ü÷g@?LbÑ?ï÷¸î@x?Q­çfÑzA?PŽ#A!@?Q­çfÑzA?ïËÂW?ð?ƒ41–¢Û?zԎ݇ì?ƒ41–¢Û?ïþdb?Y?|æ²0?)¾¼6òû?Y?|æ²0?ïÿOWšàZ?SEî«î?º]y?SEî«î?ïݖQCG0?rGOS‰Ð?q4×@Ø?rGOS‰Ð?ïÔèz°ÓÐ?¶)cxå¸?u‹Â‹iKç?¶)cxå¸?ïü‹`"5?5泸!B?;¤ü«Ë¨£?5泸!BAGN4FGL J1105.1-2600?®éœ·kç@?â2ŸÀ:ŸÀgnÀ<'•=†Æ@'ñ§Lµ@(í½\ì?Пª?ÂpŽHÌ^?óå3E§©þ@ÛÃ_»§a¿àÕd¶býü¿æ6ü¡%Ôü¿Û"ɾO†{¿ã/ýÍpa¿ïÿoì÷å¿ë¡;NŠ§ŽUNASNone?ïõǗP5š?OòTî{`?TpѤLûÜ?OòTî{`?ïðÛ15úZ?\ˆ€+±L$?^I1‹ý?\ˆ€+±L$?ïuJ<í¤¼?‡¯eI5$?'V¸d6v?‡¯eI5$?ïàµíÆV?Uß'@žÇ?oJ&ÔÒ>?Uß'@žÇ?ïÚ¶qÁŽ?t•0àω?rù¤§'Ñ?t•0àω?ïÅÚrQ×
?ˆE€w:U?}ÆäÒéL?ˆE€w:U?ïM†ˆÅ¶Ù?''ú\ì®Ù?–O.å'Vä?''ú\ì®Ù?ï|yŸöwc?{z¾qœ"×?pÌX}¨?{z¾qœ"×AGN4FGL J1105.3-0626¿ã¾7šdßl@Gß÷øʂÀ;¢HÕ[èÀ<´Ãð…8º@#P׿ïï'?³k=¯:@?çµ+ÆWh?ïÿKÚÉå'@""†âÞ?þ¾+õ&]¿ïúìšÈmÂ?ïØQ?¸§§¿ØŸ½J"ä¿êèD§¯Ý?æÑò¦{)l¿Í¶¥CÃUNASNone?îüʏõoÈ?¼"txš<ú? 3Vý9g…?¼"txš<ú?ïå-9Q¸ã?vZx'%?jÒƍJÝE?vZx'%?îm<!!'?œµ¢ Â;{?©,=ëZòä?œµ¢ Â;{?ïø9T›Ÿ?K?kiXæ]?MÃ`=3e?K?kiXæ]?ïŒÒXÒÔú?'áʕυ?ŒËiËJÁš?'áʕυ?ï rÓÔuZ?ž´¾hÆ?‡ãK¡g?ž´¾hÆ?î,Ÿ)^À?ä¡Ùٝ?­6'µ–ó?ä¡Ùٝ?ïîJÊé?pI#Uá±%?a€µ>0'h?pI#Uá±%AGN4FGL J1106.2+7303?ሁŠÈà@DüM:'£À;þ#qõÀ<5‹¶'@'Ÿ‹¡y@ãÏ¥Å!?Å^BÀïÉÒ¿»'¹5Á-?õÀ´á¼©@«'â[?×}_*ÝÏ¿ë3™àf\«¿í~ÞAê05¿—'n¯¿é[Ŏ*Y¿ïæöäÎKRUNASNone?ï÷#Vk?V àyJ&?Pý¹Ы2?V àyJ&?ïæd'#m?q¤«¹PN?i›=Xßí?q¤«¹PN?ï·2@fnì?~¿'…5úÝ?'3o֖?~¿'…5úÝ?ïé³Ð|"¶?W"äa0¡ÿ?fL/yÜb1?W"äa0¡ÿ?ïÒ¸ î7?{™Ü$t?vž¤Õ8>?{™Ü$t?ïoç2v?˜Ã•Ÿ¹³?'£‰Ó=?˜Ã•Ÿ¹³?#[$?‹oÝ "—? )jÇ?‹oÝ "—?îTßB¿½?¢'%¥)el?ª²à›Ò'?¢'%¥)elAGN4FGL J1106.7+3623?·mTþ³D~@PŠ\å´$À:|ƃÝo²À<]˽Ù@ø³"כ]@îwÐÛ?Áq56î~£?¡Œ ?ƒ¬%?ÞwÒ>Nš@m«ÿøž?ïÿÎa¢\a¿àÏÜKÅÑ0¿æ÷ôގÁ#¿âÝ­Å ˆ¡¿èך@]".¿ïþ!nÑTUNASNone?ïýo³øb?&D?@D"n?4‡9í㊝?&D?@D"n?ïøCoZD´?Pܸ۱ʛ?NòB=PúÊ?Pܸ۱ʛ?ïé³m*Oà?`ûMé—Þ®?fL"©ß÷?`ûMé—Þ®?ïýî:ä5'?ãpK×Õ]?0Ž'ãqZ?ãpK×Õ]?ïýý¢¾Â"?)0z|hÓ%?0çþÇ¿?)0z|hÓ%?ï߃'‰©.?s€ûDYÎ4?p>lFÚî?s€ûDYÎ4?ïÕPðĉî?xML"qVm?uW‡¸‡ü§?xML"qVm?ïúØ{«'?56¬VÜ8#?Dž¸r´ü?56¬VÜ8#AGN4FGL J1106.7-1742?îv;NÆȸ@C=À~à±À:xø‹—xWÀ<†]Ötì@‰ú‡;?þë'*ç?Ãì[!Ý?Ùh$¬‡³@pÀ\|@Í¥u«¿æ¤;~[O²¿¥~ŸBP©¿Ö¼ð¡=Qð¿äó;Ì_¿ìƒlfZ§ì¿ðUNASNone3FGL J1106.6-1744?çþJ]=À!?Æ\
UL`?ÐkE"½?Æ\
UL`?íÂÀ–!ƒÍ?°º¾	«ôg?±éûOÏȖ?°º¾	«ôg?å)ÞhU©Ö?µÅ9Y;P?Õ¬C/T¬U?µÅ9Y;P?îLg5)"³?‡^†â̂>?«9Œ¯'È?‡^†â̂>?Ó¡HÝ?X?È0ué')?æ/[÷'`T?È0ué')?ã"zu^sJ?ÎÎCS€Ÿf?Ø×Ck?ÎÎCS€Ÿf?Á9€r^ÊÄ?²15Oש?뱟ãhMO?²15Oש?æ8î&:°?±#Uå¼?ӎ#Ó³Š ?±#Uå¼MIXED4FGL J1109.1-4853¿îëãÚ@¹ë@%8ñ,'¦7À:eÒ(V`_À<,"d®ÖB@ˆ¿¬¨À@Ùýñ7?Ϥ4<ȈE?àãm"BJ@€˜@Ô¦@lLJ±T ¿Ê˜ÊÔпÀ'/Cå]¿âz•ÈSÁ¿â*þ~ð¿ïڋÒ0¹Ü?욉¹QÅÅUNASNone?ï«9`£0?ƒè4ÿày>?…1§Ëi(?ƒè4ÿày>?ïzª<Ó?-%B¨ÈÁ?Œ¡Ui'¿Q?-%B¨ÈÁ?íA˜…겈? ö"oÀ?µó;Ï`'?? ö"oÀ?ïF$'?€Jᡂ]ž?—;|ü׋Õ?€Jᡂ]ž?íö&`ÎF?­1Ñð^]•?°NÌ÷jV?­1Ñð^]•?ê–0–ÔJù?Æ×v
Àš²?ŧ=¤®Ô?Æ×v
Àš²?è®+çî?²Œë¡©Q€?ϕGSÀ`G?²Œë¡©Q€?é÷`í‰8?°­®×ïÆ?È"|IÛü?°­®×ïÆAGN4FGL J1109.4-6115e¿Ø,"{Wí°¿èÑØ8såÀ7C9+À9ãKÁŸr@!ÿr:Uf?þÝí¡Xª¼?£&"S¼ì?¦¯
šÜ@@Sý®(?òIK :?îT­×>?׿à'°+¬V5¿ßc? (ÿԿۛ㪵¿ãÍ®oê¿ÚpMû‹| UNASNone3FGL J1111.9-6038?å ¦iÇÕþ?Ñí¿xGÜ°?Õ¾³,pT?Ñí¿xGÜ°?ä'û?ÑðŸì*Fa?×ÉÙÎú	Ø?ÑðŸì*Fa?ãNtW?×Ü?´)؎q?ÙcQ€PG?´)؎q?×°34ÆíK?Á·Šñ56î?ä'æeœ‰Z?Á·Šñ56î?áӖ›k•?Ò,ÃÖ6¶~?ÜXÒÉ)îÖ?Ò,ÃÖ6¶~?̹¥›¹.?КØn?èі™¼ô?КØn?çšÿXÌ[?¸#G²5ý?ÐÊNgIÄ?¸#G²5ý?®Á-¦96Ä?¥Ñ}ì¬öu?îí%erÔ?¥Ñ}ì¬öuMIXED4FGL J1109.8+4406¿ïÿ¸R@O»\6À:À@æzýÀ<±*_Oð@WŸ
ÌÇC@ñ¦Ö˜þi?Äá~_¬bõ?°¥¸¶ÀF?ä»[áF×?ù¹99²~B?ì‡À=È7'¿ç"y߿éÅEŸFÅ¿î!çEôÖ׿ïÿµ¿Ö̯›Ž'SUNASNone?ïû£ú=Ö?@±î—î§4?AplˆŒ?@±î—î§4?ïmÙhLÖ¯? i"8×?'DÒô­\1? i"8×?Ó;Ã?"¼xUwí?ŒS‹BhÛ6?"¼xUwí?î䏀ÞY4?Ž6TLsÑ'?¡·ñ>…È?Ž6TLsÑ'?ïíðŸv
µ?húp)Îҁ?b`f6[­?húp)Îҁ?ë]&¬g&«?Åâì­×'ø?‹eNceU?Åâì­×'ø?ï{‡­Ù[?Œ*!tkx#?ȍ•?Œ*!tkx#?æ±o† ˜'?»S¶GþØ?ҝ ò¾ÎÝ?»S¶GþØAGN4FGL J1110.4-8023¿ïxz'9ËJÀ2aA…ÞÀ;k‰lû«ÝÀ<°±¤RZ@@!ŽUºF¸K?ó¹Ef;ž<?ÛÀÚ»¢ØÝ?éöh§‰Fe@"å$²fð@2¾/%1"¿ïÎ8<‡oË¿ísXHÕ\¿åš\!¾ì?ïgõbLM¿Ô1©ñb¿ïÿæŸÜ©ºUNASNone?ïøm–—9?HÍ$ŠF?NKŽcM‰Î?HÍ$ŠF?ïï—*˜I?eښ;
EÛ?`ëhݦÇ$?eښ;
EÛ?­"£;?†ƒ§šV>?Œ"Áh?†ƒ§šV>?ïõ—%dØ?JÕÄא(?UØÑÈtz?JÕÄא(?ïõŽ™Ø¦?V፦±À?Tâ̐¬S?V፦±À?ï¸ævŸ¢%?œ(P'Ù¡?Æbe%ú¶?œ(P'Ù¡?ïpŸ'"-Ò?½5pžOk?'ìºE·?½5pžOk?ï̾"	n?zBHN¡Ad?yñ ÂÙá?zBHN¡AdAGN4FGL J1111.4+0137¿á<Sy5X@K€`VìÕÀ;'‹®ŒÀ<bjáö)½@û}9f©@XdàTi?ÊÍG›õêR¿=ugÓQ_ê?˜ã#¶V5?ùðrƒÖ
é?ïîtÝw"â¿ëqBb{[¿è&Ï!»¼"¿ÔÈUÚ'(c¿ç–Háñ!@¿ïù&A³(·UNASNone?ïüæx—+?/žÃº?8Ì@ù_Ó³?/žÃº?ïá†êâ®Ù?tÛlœé3Ñ?nyUª¾ô?tÛlœé3Ñ?ï⾒¼™?hYZ¢–?mAm[>¿T?hYZ¢–?ïÓÕâ?\]?ïo<?v~•x¿?\]?ïo<?ïýA½Ë¹8?2È*9|S?5ò7_"¡?2È*9|S?ï"ÞòFô?'vV»¦ô?‹~µ¯Ó,?'vV»¦ô?ïÀМ²u*?R%º`?—±h?R%º`?îµpÁ¢æä?'Ð6¥ÕÅ?¤¨óç‰_¼?'Ð6¥ÕÅAGN4FGL J1112.0+1021?Ô#?ò©€@N›‰
Z[–À:²˜ˆøa¦À<beÀN9I@ž¡@W@	z¾A?ÈlxÏ¿®•ûÝå©?×¥_ yˆ?ÿã&«esø¿ÝÏI~Ïø¿éu¢¿<_¿ïaß¹8›R¿ë"ãw3=D?ì.rýMž¿ïÿÒ³–šâUNASNone3FGL J1112.1+1034?ӂ|$?µÚ†‹lQ¯?Ž×‹¢‡?µÚ†‹lQ¯?ïñX¨–?P?jÀHVœI?]N®{‹a'?jÀHVœI?ïlaL~"?ŽÏ°uáÖ
?'sޏ'Ó?ŽÏ°uáÖ
?ïÿe/Û?
¬»}°q??±¾|9?
¬»}°q?ïÊ=)Ååí?†Û¾¢òÇ?zákݽº?†Û¾¢òÇ?ïœÈéúkR?—F	y¦_?ˆÍŋ³ÿ?—F	y¦_?ïö¦?–16ˆòN?!?èÅQ?–16ˆòN?ïì†J Nn?hÏ9°óè?cyµº•ÊN?hÏ9°óèAGN4FGL J1112.2-6055¿áVqKN'¿Õ8;SéÀ8¤à·e\{À:)1™Õÿ{@ 
y#ŒÈ@­'hr°!?ʚ_,
u?ÓOW xEŒ@T>S!æ?úyLò÷ÙÁ¿îg8¿d?¿ãÎ_ã¯+¿Ôv§ý	«z¿æ¿£ƒþ&â¿éR½g)/¿ï+4+€·KUNASNone3FGL J1111.9-6058?Ón
–ÿ-?Ñ|õ.?Ù_?æ|Hú´€j?Ñ|õ.?Ù_?Ç<¬"Ú(f?Á'ú8ôEë?ê0ÔÚÉuæ?Á'ú8ôEë?ÕÙfþç§?´ÄðÛ?åL€Œ,t?´ÄðÛ?Ïά¿µ?³Mú¥´@J?è~Ð>?³Mú¥´@J?±ÕƒÕÈ?·+ý¹¨?íÅO…N^?·+ý¹¨?Šåèæ.±?hJ?ï"h_dêe?hJ?ÂÕþˆËYõ?«~£¦¼+?ëJ€]Í)ƒ?«~£¦¼+?v@FLQ?pÕÎi2?ïÓsӌZ?pÕÎi2PSR4FGL J1114.6+1225¿çi¢Ñ%Ìî@O}Ëݹ"À;dÑ~uYÀ<›ç+ä<@g}ÕÃÁ`?ôFâ!ȧ¤?àþ'î?ïÿqÐ&ô@Ø®$kT@I§¾ËW?ï<m¿ ;à¿î»+à-§®?Òa¼­ž¿Ö‡KMÜ+å¿ïÿójÆGx?ä"e}2ZÆUNASNone?ï±ÆˆSåÊ?'s¥™K"æ?ƒŽ]ìfe{?'s¥™K"æ?ïÆÑIŠ§?'/Ñmµ)?|—[™DŠ?'/Ñmµ)?î57´™œ–?šÛu(˜?¬¬"³Ò¢?šÛu(˜?îâ?eEª?…éúµ1?¡Ü	©ªÏ?…éúµ1?ïmL-Íe?™!ƒìáÁ?'VzA+ò·?™!ƒìáÁ?ï …£Þý?¨¼‰Bù?›ïK"ãXS?¨¼‰Bù?íåï$)nÓ?¢Pî0¨(?°Ð†Ýj®é?¢Pî0¨(?í¬4IïÉb?§áº?{×?²ž]°´î?§áº?{×AGN4FGL J1115.1-6118¿ëˆñŒ}Z¿â-tw¡!MÀ8D~ïÊ'×À:
ž¿s@ rHqß@Öº;А§?³¾R`Ÿýâ?ª‹~g¨Ê?ùãòhgÈf@"³U?ìŠ@Ë¢*b¿ãÆ
`:Ó;¿ẩæž/+¿ç'¼£n¿ä˜êýºU|¿à5몥çUNASNone1FGL J1115.2-6124c?íK0wd?¾Ÿôo±œM?·'å¦Qd?¾Ÿôo±œM?ï'þçôh?¥€tˆ×Ä;?œÍÀ";?¥€tˆ×Ä;?åú)ÚD»?¶BÊNŸ?Ô¬KwøŠ?¶BÊNŸ?í°_"F?›…˜æ]›?²}jªN?›…˜æ]›?ê3ú¶óz?Á῔Sñ?Ç»0$2?Á῔Sñ?ëµ"rVñ?É'²Þþ?Ãù+v6¤=?É'²Þþ?çŠPoq?¼aMU{æ?Ðë_!×ç?¼aMU{æ?âW@˜˜à?¿ó>ïT?ÛQ~ÎÎ?û?¿ó>ïTAGN4FGL J1119.9-1007?Ü:tw˜ŠG@GQµc#»ÇÀ:ë浬×À<b¢Œ‡b@N-ۅw?ÿX×1ª?Ñ+û›í0ð?΁ûWϟ»?üöË #÷@	^0;;X?¼äaئä¿ëY:>b¹¿Ã;Û"zÿ%¿á¦ßîÁ¿èRàýÜ9Q¿ïÛ`í*»UNASNone?ïýc5·ûb?0†ûÊmòy?4æQÆ6o?0†ûÊmòy?ïó"êe¹î?Z'œ²K??Yº*äÕ4)?Z'œ²K??ïÜþ†‹Óf?ol¬ÇåÚ?q€¼³7?ol¬ÇåÚ?ïòRE²è?>Ër08ƒ?[Zßi›pÓ?>Ër08ƒ?ïü£ØÈê¦?8¹!÷á¼?:á:¢ÜùÉ?8¹!÷á¼?ïÇÉðÏ`{?ŠÀtq8sÜ?|®ý.l?ŠÀtq8sÜ?ï¾ÍtK?€ÆLçš‹?€L¢ík­í?€ÆLçš‹?ïÖ_±| v?^×}Îä‰j?tÐ'#s5K?^×}Îä‰jAGN4FGL J1120.0-2204?ïûÅØ´.@B(ÂzÀ8Ígi›¥
À<ø¨ê@Þ}˜19´?üæ+ÈÛ¦"?«µÊ|»gu?Þäµ—&"@/êjP
@•'æxðW?ïùÙ?¡Ö¿¶UŒ_°zî¿Ý£¦ï¿è"kdÒè¿ïÿûbâMh¿ïæó{?UNASNone3FGL J1119.9-2204?'à,h"Z?›'.èi?ïpþœõæï?›'.èi?Ãý¤AN?ÀŠ¨˜˜›?ë:À–ï¬\?ÀŠ¨˜˜›?µh̺	}?¢í¨dž9?íRæ|ÿ¸?¢í¨dž9?ZPᨩ½`?VM׺–³?ïò׏Ϫ?VM׺–³?v‰×؍+?" Kêƒ#Þ?ïÒìPm":?" Kêƒ#Þ?¤âŒöù£?¤ÂÝÀÒýð?î±×?¹Ë¶?¤ÂÝÀÒýð?¡hµr©oï?˜õåþT·Æ?îét¨žoA?˜õåþT·Æ>ßp›X7>çt-C#?ïÿðH'2>çt-C#PSR4FGL J1120.1-2645¿è}w$#Ì@?Ï>$þ½
À:GXS~,VÀ<_'fÅ0÷@÷´Lù,ý?þèõÝgNÄ?º/÷¿i·Õ?ƒlßHǼd?ÊaÁ'ýö@­¨ñ{Wå¿Ù‹Q¢Š$¿ã5æzyC¿Ü팈†w¿ßœ7£Û;û¿â6þ™Îs¿«P'	ÚoUNASNone3FGL J1119.8-2647?ïþÉÂk
?
²É?#câäú]¯?
²É?ïõFNK›?X!—;²¾ó?Usc¨¬o?X!—;²¾ó?ïú9)l_û?OA¾×Q0ž?GYäò|³?OA¾×Q0ž?ïýixGB? Äg2¨Å?4´>iÃ9«? Äg2¨Å?ïþ^ê"~š?z¬k<?*Z€C¶»?z¬k<?ïÓ¥»¤?z}¥"DA?v-sp¹?z}¥"DA?ïüeñmãU?Pa¬ä	ƒ?<Ðv[dj‡?Pa¬ä	ƒ?ïùLMœ§&?;ûFx5SÐ?JÎÉK÷£»?;ûFx5SÐAGN4FGL J1122.0-0231?ì.·+¶ù7@J¬wFˆzÀ:õQ³PúÄÀ<Cb?8È@Šx•½ìà@c줩(?½É¹ÇâWN¿»é\`º;6@k:á}]ú@ܨX¤0÷¿å•b'¬K¿å6fœí¿èð«Ï&C¿åé'yâ¿äû9âyÝ<?Ö¶›Ø'UNASNone?ïü€Åžkw?1Ia§s¤£?;ùÔ"Ñuå?1Ia§s¤£?ïÏû¶¢Çs?|"BÍÀtÈ?x$"f?|"BÍÀtÈ?ïÜޑ+#?s}Þ
 (Ü?q·oâ~?s}Þ
 (Ü?ïëöà¾é'?TlYµŸÿÐ?d	-Ø®j?TlYµŸÿÐ?ïòáÖ8E?ZN°¹²
?Z<SyÃö?ZN°¹²
?í}†]I(µ?ºìrm'ï?´ÍþìX?ºìrm'ï?ï|Ìüië?Q¹Â?;e?lF]&«?Q¹Â?;e?î4ú49?£½H©à?¬¾?=Ér?£½H©àAGN4FGL J1122.2+3926¿äçaââҌ@PðváÞ¬ÉÀ;(à#Á¦(À<'i<Ú{â@#³—œ"@[iQ;?Çúj"2°¿¡C!£ú׳?ÖQå&µÌ?ü¾#çÈe?Ö_#Æ®¦¿é¢²G‰
¿çXl"h	Õ¿åþ‰¾]¿éPKý"z¤¿ÓUG¥[ÕUNASNone?ïúBêòbð?Aø`¼V??FôUçý?Aø`¼V??ïêüE¾Ù£?j-z¬*€?eº-èt?j-z¬*€?ïڞeä?lZ6Q}¥?xª±['Ï?lZ6Q}¥?ïÛöÅ]†ˆ?YuãN?rpÙ#û?YuãN?ï÷E˜W?O¾>ZÅ>?QtÏ@Š«µ?O¾>ZÅ>?ï?(	'?'™¼6ùý?Œ06d?'™¼6ùý?ï©öÎÓã?ƒ`W¹'dù?…'LD(e?ƒ`W¹'dù?îva)ˆ?–¾ùœÛå¼?¨žoF}˄?–¾ùœÛå¼AGN4FGL J1122.4-6237¿ç¹]¤Jø¿ø"ÊL¿ÌÀ9SdžJÀ;
¸ÜU
@ 7~ä6¡@Z¨!ò™?¾ònGx? ÜñC_âO?æ)Ïqºû@I4ý7Σ?î²:zOQw?ïàß¤jٿ媚rÝm.¿èÇ)Š=D¿ÍÀ‡Y¦¿ë	c@—ëUNASNone?ïòÓ±aˆ?b5à¬9™©?ZXÏŸ?b5à¬9™©?ïÝSÐ
M?{·ˆ™¡d/?qVx éÕª?{·ˆ™¡d/?ï.‰–ÓQÝ?"pœ&6?š.Í nZ]?"pœ&6?ïÕ¹}î ?b‡‹èg›7?u#A_•Ú?b‡‹èg›7?ï|':-+?(¶,¢Jm?}mÝáė?(¶,¢Jm?ï$Xÿ?«¼3>?›~4÷(6?«¼3>?îjŠñÉ?¤IŒÖ†—±?®‰Wax±f?¤IŒÖ†—±?îþu†"Ú?"¡"8&z"? §"B'?"¡"8&z"AGN4FGL J1122.5-1440¿íÁНòl@Ezã`'À:‡ànj@æÀ<N&äpX@Þ2>k @|ÿŸ‡ð?Â|ãUzZå?°Bü>l?çu	Ar;1@ꖧ 볿ãOµqfu¿âøÈÔÈ(¿é=ß>ir4¿ìåþÌú6¿ÄçxŸ£ô¼¿Öԓj«o…UNASNone?ïçËL
?¦,Ýå–Ñ?hü4¯º6U?¦,Ýå–Ñ?ï🋇Cg?alD·kô?^ÀèÞ;b>?alD·kô?ï³t?(?'¶û>L.h?ƒ9~çg³é?'¶û>L.h?ïùäƒ*tü?6q¶Pé?:?Hmô.9äk?6q¶Pé?:?ïÉÉY±R?ƒÖ5cúO?{SŠ?ƒÖ5cúO?ﬓ¹Û®g?Ž>у4f?"ÛŒ":?Ž>у4f?ïQ¬\·2~?'nÏ@šyé?•Êtl‰L7?'nÏ@šyé?אּô:`4?~c*
ü?"ÓÂÿ&b×?~c*
üAGN4FGL J1123.2-5111?ïרcó@"š{9&À:¸ÕŸeæÀ<RÂ&@»¡iÍf@NeÙx¬º?θ©?Ñ&?×8´|sîå@·±ÚØÿ
?ü|h±D[¿ïuH¡¯g·?ïé$ò'Ð)¿àL"b¥¼"¿à2kݞ¬(¿é4èªxäî¿ïÿŒ	ß}UNASNone?ïÀ*D¢s?z
ÉÅòð"?êݼ°¶F?z
ÉÅòð"?춾B›[?¹Uc>I?ºJ
ë%''?¹Uc>I?ï0#x?¨Žþ*ÕÑ?žyûŠ§e?¨Žþ*ÕÑ?îE.K–§?ˆ¯êPܵz?«­O¾c?ˆ¯êPܵz?î­¥í1h¥?žhvÐD?¥%¡,éu®?žhvÐD?ߢÄ"Öf?ÑÚK¼}/'?à.ün"Í?ÑÚK¼}/'?ëmÆ4µÈ?­¹¡E²?êHç-(á?­¹¡E²?å2
ÂâÏT?µÎ¦8/éŸ?՛êz:aX?µÎ¦8/éŸMIXED4FGL J1123.8-4552¿²¶1¹bA&@,­kD¸ÃÀ:2ϾÕÀ<Hóµnâ6@Œ¾A™¨]@ÜOÜ·%œ?»Ýظ¾M?±g?Õ-'?õ/$*³Ê@qI^BÖi?ïùJYPԿʓÂjU%¿è-YŸ®†'¿à×ewS´¿áÙ[ñ˜^0¿ì"Áœm	UNASNone3FGL J1123.6-4558?ïû±©R@·?3
ëôw?A9ZbS'g?3
ëôw?ïãÕ¶3?uMɶ¾ª¸?l~*nè¼Õ?uMɶ¾ª¸?ïñ~)ÖN?Z8<©Ëã:?]ð3w?Z8<©Ëã:?ïè'p©­°?JaîªåH?g؏ùø?JaîªåH?ïöú*܀'?HÑJ—"ÿ?Rª²Ô?HÑJ—"ÿ?ïas1âû?_ã¡lÐ?"љڰ?_ã¡lÐ?ïãÑEãB?w\É.Z¤ó?l.üü=î?w\É.Z¤ó?-Ž¥í?teùºÍA?‹Ÿt'°Í?teùºÍAAGN4FGL J1124.1-1203?ŠN÷`ÿ\@FºY!…ÆÀ;+Ÿ'xÀ<•®Ðbƒƒ@Vï|úýb?ÿ!ƒ†Ý?Ü­$ÜtÏ?ä¶öq@"恩¸Ì@ïZÎy¿ïü!~|?ïÜ^o÷ß ¿Ù€¬ã£S¿éCa(¹Þ¿î-‰Û¶tœ¿î¤Q]똕UNASNone?ïî2…ŽIÚ?w¯«>0·?aÍzLš]õ?w¯«>0·?ﴅr	 ª?ƒ"ó³¾£\?'Þ£pQ[›?ƒ"ó³¾£\?îÒ`Yð¥?Žþ]¾wš?¢Ùúkm@³?Žþ]¾wš?ïA^;?'
"wDl?Ÿo×Ïn«?'
"wDl?ï¯ògwCÀ?†ƒNPڗ?"f!$ ?†ƒNPڗ?îÑfF}_I?©ëpu峙?¢é›™òt?©ëpu峙?í;OøÌì?¥$º‡kgÚ?¶%€;Pmi?¥$º‡kgÚ?ëQû<÷­ ?«C1iÒ?¸!K?«C1iÒAGN4FGL J1125.2+2557¿à…˜¦yk@Q­LD|0ÓÀ:+·=ïOÀ<€¼ÈrÊù@Ùÿ°yÛ@ð@|ÇÑ»?ÄàðZÆu?ÕÁ~gô@	¶§[ùûÚ@rZûÏ×?ïýË<©Ôz¿æ	g½~{0¿é–¹èîl¿ê""½¿ïý²GæHŸ¿ÓО¥2UNASNone?ïçU¥+¦«?eð))aP½?hªZ'`ÕÚ?eð))aP½?ïN0wl5?¤Qœޕ?–9ñċo?¤Qœޕ?îüCm'?"®
ÉUü? ;É0•\?"®
ÉUü?îñæ=Gof?"Â"¦âï? áœ-@ז?"Â"¦âï?ïß­ýSÓ?tô­G"•Þ?pw)'C?tô­G"•Þ?êu>U¦$Â?Æԕ_ŠN?Æ+©gl÷?Æԕ_ŠN?î ¸ (¦?¡'ä9I#•?­÷$|E§¨?¡'ä9I#•?åßü¸Uz?¶/gn²?Ô@Uå?¶/gn²AGN4FGL J1126.0-5007?j``@$ìܨââ¹À;E²à'|oÀ=–"TÛú@˜Õ1 6?ÿoB]r¡Þ?Ó|
}é?ïG}½›¢@ÇVO—î?ý)ºËÃ?ïû²}ì¿æ5‰2C¿È'MÅ°£Ì¿ÒՖŸê³¿ïþÂ^§U¿æU/þËMUNASNone3FGL J1126.8-5001?àˆ6›P0£?Ì°âÏ¥€?Þï'É_ž»?Ì°âÏ¥€?СìTã˜R?Âï4­Ôž?ç¯	Վ3×?Âï4­Ôž?áÁ·-[á[?³í-íp}¹?Ü|'¥H=J?³í-íp}¹?ԃXQ£?°	S'ó¤?å¾Sö×.?°	S'ó¤?ÖÌ'"öJ?ÐΐWŒÀ?äó™ì6Û?ÐΐWŒÀ?œ,V΂X? Lº
nÆ?ïI§hå? Lº
nÆ?×'ûlG{ë?ºV{wD°?älIÜB?ºV{wD°?¤uÇe+i??'ð0#̎?‰vO¬?'ð0#̎MIXED4FGL J1127.9-6158¿Û;_¾Ú.¿åÁ¹óêHÀ8ÿÁõuüÀ:²ÿ%¿­@Òg°"[<@–øAŝ.?ÁÇHhújj?֚ɚh@ߧÃ(]?þk§ùÈ.?ãů¢›¿Û–­@•ql¿ã×ómJ†¿éå9àÌ^¿ì¼í[¸{¿ïòÌ&°nUNASNone?ІWoJ-?È$Ìpºý?ç¼ÔHZüj?È$Ìpºý?ÈrÀ¯æ•©?¾\#õÜ?éãOÔZ–?¾\#õÜ?Ö¤ Ya?³Kq8¬Ë?ä­ïÓs@P?³Kq8¬Ë?֑ÍÇ7{[?°cÏ؎ڠ?ä·dBR?°cÏ؎ڠ?é"¡s5_?ÜŽ)ܙà?ïx¶ê¯®%?ÜŽ)ܙà?‹Ž5@]ñ?Ž=-Oo?ï'Ç*ÿæˆ?Ž=-Oo?¡Mã`%ô?"íOâ?îë.'µÐ?"íOâ?‰3«Z	¬i?u{eoO'?ï›1Rnÿ?u{eoO'PSR4FGL J1129.1-5230?ÂüÖ#|u¶@ ´Ž:!dÀ:ËêpKÂvÀ<BW¿¶n@/§J\D¤@#Êŋì?ÁÊZÒbä¿¢E›ÚUe?áKÌQ|ÊV@
ájCÒ ?é|=}¹ê¿ÃJ&¿²]
¿ê……t¿Ù-Aª‹¿ßEqcÅwC¿ãñ" Ü.UNASNone?ïþ¦ƒâÎ?¥ó0ˆ};?%—¾†±ØF?¥ó0ˆ};?ïè þ/ú?v¦#?góßOf-?v¦#?ïóÿ«
I?YšjUWu?XªhÃã?YšjUWu?ïþµÁÝm?´%~Ë?$£åNŠñ£?´%~Ë?ïúþ>Q?Jk¤»Z=?EÀfƒÿ4?Jk¤»Z=?ï9îŸX?¥Â…ƒß‰m?˜Þ"(¬™?¥Â…ƒß‰m?ïï¨xõÂ?kâ-Ü°
Z?`W‡½¯f ?kâ-Ü°
Z?ïú_÷%T½?:l&µœ'œ?F€$dК{?:l&µœ'œAGN4FGL J1130.5+1400?ÏŒBn¦@PÁå!WhÀ:È£öꭈÀ<r5r
	@a
þw¥@îùûA?Äm¦ß'm?jF/Ä{µý? ÕÇóE:@ýClç4¿å¾¬#¿æƒŠT'¿åGxÏõv9¿è|üÀZxœ¿éÒŠÝ>4¿ïmè jUNASNone?ïþ†Sý¿D?&œ$C8€?'šÁJ·ï?&œ$C8€?ïö@²ˆäý?VÀÆHj"A?S~›ð¶j?VÀÆHj"A?ïì‡hGDÁ?Z÷
Ngµÿ?cx—Çه>?Z÷
Ngµÿ?ïû|²¥{œ?-£)ê7w?B
5GûÔª?-£)ê7w?ïýÞÊü5?*£[³ú@?1	¦.s©Ï?*£[³ú@?ïѵ†×l…?ƒ1¬)"?w%<"{‰h?ƒ1¬)"?ïézˆv ?jþSýã$?fà…Rn®?jþSýã$?ïçpõ`"À?Zi"v¬›?h
½§Ï•?Zi"v¬›AGN4FGL J1132.1-1448?ëMߏzº@EgÀ:÷nªØ†>À<ræY¶U@ #3ºÂ‰'@¸ù±1f?ÐB¬©—?¼¶ðÂuZö?ñ åRՏê@3¹ˆw]Z?¤àA@{?ÒD4¢Éî÷¿å.â q¶¿Ñ²;{+¿ßö'þ¢ˆ¿ïþù:!EUNASNone?ïþþh%XT?ÁµIYß? vrž'?ÁµIYß?ïó"ÐNXö?Z2áæѼ?XØ_yK"(?Z2áæѼ?ïôÌY´?^Íi Ç§?VgN-‹"¨?^Íi Ç§?ïø£ã¨/?1 ,ÌÁµÜ?Mppß"°þ?1 ,ÌÁµÜ?ïÿk'Ö ?Gi‡^ë?›É{4"?Gi‡^ë?ïÊ,¿¯5–?‰\
ÎÈñ
?zé ']!?‰\
ÎÈñ
?ïö¢BNrî?aûßK·ÞÞ?R»{½ÏҐ?aûßK·ÞÞ?ïáEÅ'‰?^¿\»†˜$?nºô(ú~Æ?^¿\»†˜$AGN4FGL J1138.4-3555¿å(ìD%7·@8¥à?pXÀ:Ì<Ý ·À<{(7V®b@ؽ›×a@Bý@27?ÐâÛ¬äz?Ó(.rýN@ä%C†gŽ@`'ÿ÷q'¿åív% Jù?ïý»ýœ£d¿âRÞt?¿âw8¡Jr¿ïú?–më¿ïÔ. §TîUNASNone?ïèx¦ý&Ô?‹qæÁ"q/?g‡X¿€Ô<?‹qæÁ"q/?ïÜíüÈ=?r´7…upÖ?q‰­¿j]?r´7…upÖ?ï:î#<MÂ?Š"R3€?h?˜¢;ŸUÀ?Š"R3€?h?ï®V\ƒ?fgP rÉô?"z8*hß=?fgP rÉô?ïçoԊl'?e¼ÉȐâ?h+¨m¦…?e¼ÉȐâ?ïuà?™ê¡êŽ
P?'CÿÛ®A:?™ê¡êŽ
P?î\À©§ž?ž6êlÐ ?ª3÷á.?ž6êlÐ ?î?b8'?˜o+§·¥?¬	ßî5ÔØ?˜o+§·¥AGN4FGL J1139.2-6247?ëÇY5¸¿ñt¢iKôÀ8†8<‡oËÀ:¿mã2ià@uòœj.r@¸*Ž;?²î	!U©ï?È3<mn˜d@þ¼ž_ç?üQº¥WèÊ¿î¬B®Ûö?ì"ß(#½¿â†¢F†¿áë,i–¿éH§8¾o¿ïþç àö%UNASNone?ßÛ²
-åì?Ñj©µ-'?à&ùi
?Ñj©µ-'?Å_á~¬û™?»^cD•R¯?ꨠTÁ?»^cD•R¯?âCŸþsÊ
?µ–þ
ÿ¯Å?ÛxÀkå?µ–þ
ÿ¯Å?ÙãxNµ	?²LɊI°Ó?ã|ŽCØ¥|?²LɊI°Ó?Ÿ!éV»ç?²nNèˆy"?ï÷ÀìCà?²nNèˆy"?ŠÏÕòŽž?Œ&?©+Š?ï"À¨Š8?Œ&?©+Š?Ɖ~VФÑ?¸kWÜ'?ê] jKÖÌ?¸kWÜ'?–J«£F'?…ëÙ5™2?ïMª£L[?…ëÙ5™2MIXED4FGL J1146.0-0638?àŸÿ¾D@JZ?>pÎÀ:b=ç™À<M·½q7@!'Æ¿¬?ùð'Iü?½³TUª?½`OKÔ®?ý\ÄÞÁÂ?þï·]yÙ¿ïý?Æ¿l'?ïAJ·æ¿´|£ÿùõп;«·ShÞ¿Ø-‹¾åƒ}¿ÜŠ"¾@BUNASNone3FGL J1146.1-0640?ïýfWDVé?%wÁ's™|?4ÍDɤ?%wÁ's™|?ïÜ,Ɍ¦l?rÅ!EÁžz?qé›Gk9å?rÅ!EÁžz?ïðÎrÌ?V3˜EÍå?^c…ýèq?V3˜EÍå?ﮆj£ô?iÚ3Èód?"z\¿ý?iÚ3Èód?ïø»	£9M?Cì3S?MÚ:ª}?Cì3S?ï|YâõX1?–RÃW"M?tÝå]Ü?–RÃW"M?ïèÏ^pT?q]^åô}?g0¡¾KÚ?q]^åô}?î½NÊ4ä[?'Xc@¨?¤+\±ºU?'Xc@¨AGN4FGL J1146.0-6822¿¯IMñfÿÀ
[>ê÷ZÀ:lF"
qÀ;Àê×yÎù@¾§ðõK@W^ FÇe?ØÖrÓ\3?Õ'H㞠@¿ìTR@ã´2!:b¿ïûì?XÛc?ïÿ©Î›&¿è0Ç}Øró¿â±ŸŒ¨¿ï䍞8º²¿ïÉ™"{UUNASNone?ïUU–yB{?›Þ£Ü5?•UM0×°£?›Þ£Ü5?ï.–ƒ&­?£z{ñ?š-/¢ªÆZ?£z{ñ?í"集ü? <øoB!?³Ø³%ú'? <øoB!?ï\;?'?þZ©èÉ?Ÿ´}y3»?'?þZ©èÉ?븭âë‹î?¾K
n²©û?ÁHtQÐF?¾K
n²©û?êíÔ¥šj
?ÈðžEÕD?ÄH­i–W×?ÈðžEÕD?æ%4='†?ºáÞõÌÓá?Óµ—…±ôô?ºáÞõÌÓá?çO.
¡»ô?¸˜Ô®µ¸ô?Ña£ê¼ˆ?¸˜Ô®µ¸ôAGN4FGL J1147.7-6618?ÒV¨/Àê^ ŸGYÀ9ì¸ô¨´À;{oɼw@ÖÙ¶?A´@…æÿ}ú?ÌÞÏÄ#?Ò6Á}cX@-F|¼A@ç;¸è¿?椔3ÿ
?êÉTýÞ<·¿å'ÊÞ
6æ¿èæRkÞ¿í¡]¹»¿ïüL·h·yUNASNone?ïbÖ¡·Ë3?§w"Šä)?"¥+ÇNË¥?§w"Šä)?êü)´âÓÓ?¿‰¸‡è¹Š?ÄY,t°µ?¿‰¸‡è¹Š?ílÚ(ªï?Ÿ£¼þ»–Ë?´™.¸ð¹ö?Ÿ£¼þ»–Ë?êÍݗ[?¢1…ÆzO?Äȉ¢'Ì?¢1…ÆzO?é»LÒõ
'?¾Áä¼W´?ÉÌ´+É»?¾Áä¼W´?ÙîRrWz?ы¥N`½?ãtÖÆÔC?ы¥N`½?ážU:Ä÷ì?¸ZÍñ:?ÜÃUŠv(?¸ZÍñ:?Ðð¦€Ýµþ?²§ÉÉã?燬¿'%?²§ÉÉã	MIXED4FGL J1148.2-0029?ɛ»žãA@M<=îx@À;+&ø'MuÀ<‡·ôÎs–@֛3w¦«@BúP"–J?ÆHàÙôþo¿˜à>ˆk?Ñt¶`NÊ=@€èÚ™ô?Æâ=¢Lñu¿Ý"PÄé~‰¿ßÃ!R`¿çúy
2ª¿á\ ý¦‰l¿ïÿå]½JyUNASNone?ï÷üðùIO?d¬'€~°?P§£¶?d¬'€~°?ïïWÓóÕ?byçcQ`?`ñ¨Ž&?byçcQ`?ïÁ!:Ýï?û-&¹†)?o9`D˜?û-&¹†)?ïðY3Drm?Cô-N@?_M™=a¶?Cô-N@?ïòÁý™|?TÜê.6$?Zä|%ÉGò?TÜê.6$?ï¹][r8ú?‹µ#ÛêÄ?¨©1àr?‹µ#ÛêÄ?歷àèQ|?"†d',Á2?†\Ǹ-0ú?"†d',Á2?ï"ü"™2I?y=""Á¯?ŠÀÚÒÔ5½?y=""Á¯AGN4FGL J1150.1-6324?属SpH¿õy€TN5îÀ9·Lz,	À:öðf/	@:Ïzüö`@_¤?åÉ?φbЋž?³Ì{O,8?ð_zNz·V?úH'ëÕ|¿îóÑôSúS?îc2Õ?b¿ãå˜u­+G¿ìbXŸÔF>¿ÛÈFøã¿Ò…(€nzUNASNone?ïø»p·€¾?U"þJ†Ö…?M=\C5?U"þJ†Ö…?ïXŽ¤ž?Ÿ	«þµ£?"î+g\?Ÿ	«þµ£?îR¥vLJ"?žü Ofï?ªÕ¨óÑË?žü Ofï?ï|ûàš?{ðõ_¸ÙB?`ž‡\X°?{ðõ_¸ÙB?ïyùA䕰?šI"0"–|?À×ÃmIý?šI"0"–|?éï¤PE¬?͓7·ž´®?ÈC¡n¾éN?͓7·ž´®?ëñ.KËc?°y{\Ñ?À;FÐÒsˆ?°y{\Ñ?è=´ ¨xý?¾6Õ:jÆ.?Ï	-}^?¾6Õ:jÆ.AGN4FGL J1150.7-4613¿ïñVÁ¥Ô@.ºp6ÉÁÀ:†Æ÷ µîÀ<i´g{9\@›Ö_ȓ@"i7Ñþ?Â&Œš?¸[GàzÏ?÷êg²–À¡?ú%[Øï?ïôÿ¼
aè¿åÊsbοãîð®Se¿Ýñ^|¿åƒ^)+¿ïÿÅbu@UNASNone?ï÷¸)7íé?CR·k­¹­?P­Ým%?CR·k­¹­?ïm¥Öˆ¥?—x6f|2l?'KE<ŽëZ?—x6f|2l?ïá"9ø¹?qð÷æ_QÁ?nÝçG?qð÷æ_QÁ?ïd2RT.?rýBü?"yµÄ4²@?rýBü?ïê§vbC?]Âfÿ!?eàX©:$­?]Âfÿ!?ìÏPð)ëƒ?¼ƒ£¹?¹…xú~d?¼ƒ£¹?ï¿åøå&?ƒ~ÏÔÂ!<?€ÃöϪ?ƒ~ÏÔÂ!<?ì á¯æj¶?¡æƒv$q?¾øò€ÌªN?¡æƒv$qAGN4FGL J1150.8-1905?âÄÅö2f@DÁâCV—À;Çj
_ÕSÀ<Ýû@ý @"B;ë¾'?õò…=Ân?Ùõð"?Þ¥*ÜÍuê@Ðkæ'ø?ù	E0‹¹¿ïÿ+YJ1?ï)·¿Ža¿ï±	b¦é?ïþmÄ(¹]¿å¥;X›¢ˆ¿ÚD÷€Õ}uUNASNone?ïú¥C{L?[~lû§?Ek®»ø?[~lû§?ïrRݞ?Ÿ—<òúˆó?'µ½G»ÙÊ?Ÿ—<òúˆó?ï•Q¿v‰/?'
Ž|ĝ?Š«,¬ˆ?'
Ž|ĝ?ï©áV?y	ãÐì¹?…¾g†r‡?y	ãÐì¹?ïéjÙä?f^ª'ãU?f÷•çH$7?f^ª'ãU?íÔRÜ,!'?¾}&­?±]iç%ð?¾}&­?ïŽ}X	E=?Š°Ñµ
?Œ`ªm ´?Š°Ñµ
?íƻ¯)?«¿ÖXâ{R?±Ê!íÀ¬;?«¿ÖXâ{RAGN4FGL J1153.7+1857¿îAÞÀ¦_@R›ÓíR~RÀ;QÓq+¼FÀ<¦?|ÑÔ@\GŠ®@²9{Kй?Òx‰éù-~?Ãyç!·µ¹?ñJÀ²¤@Gz½áM¿ïÿ*LÚ¤&?ïâ¤.™p¿á¯ÊÈæŽ?¿âzó¼$ÞÝ¿ë6#það5¿ïÍ	žs`UNASNone?ïø78Ò?HüÞ83:þ?O#•¸k¥?HüÞ83:þ?ïï³'ùÝì?a®oì+t¾?`LØ ??a®oì+t¾?ï [žõ?'@ Ð¸ÉD?‡é;˜\'¸?'@ Ð¸ÉD?ïà*sWKÒ?Tª®Vúi'?oՌxÝÂ?Tª®Vúi'?ïÜ/jÀ'?o§C1,Ç?qóhg|vØ?o§C1,Ç?ロ#åëà?‡f£ÁôS:?€Y6öè?‡f£ÁôS:?ïސ2v?•JÓJÛÀ?ŸD-òЙ??•JÓJÛÀ?ïVš'ÖU.?…Nû-
å?•,»¤ö6?…Nû-
åAGN4FGL J1154.5-5952?ë']
¥¨ú@ÀµgUy¯À9ۅèÜÎÀ;gcRµ¯@íp¨‰¡@¶*ä°a?Ê«r«fÌ?ÞÅè¬ý#­@Â¥Fv@Ñ)÷öP?ïÿ«|,Ò¿ß¼ R:Š¿æ3ªïê¿í'›h¦²‡¿äϵù¿ïQ(l/ÔUNASNone?î±–.'I?¨`uÖF?¤îòÒm?¨`uÖF?ç÷$ËÖš?Ç$‡5‹I—?жhSÈÌ?Ç$‡5‹I—?쵟ɔð?¤Ð&a}CY?ºSñ³X?¤Ð&a}CY?í/¿39ÆÔ?—yýñ'¸?¶'f1Éb?—yýñ'¸?ìŽyìïƼ?¹ô%<‹²·?»Œ0˜Ê#?¹ô%<‹²·?¹/oM¸?¿FÅ-¾v•?ìßZÎy?¿FÅ-¾v•?ã—F°5î?·Š"7íȔ?ØÑrŸ•î%?·Š"7íȔ?ÕM¸¿"Å?¼:¯9¥#w?åY# v¶?¼:¯9¥#wMIXED4FGL J1155.2-1111?ÕOÇÿï @Hª›(ÂÀ;	)ÿ­ËÀ<ˆ‹y¢ƒ@!õäs2?øRñ>œ?ÜXiwÿk?ÔaæÕw–?ù‰,£Ìù@lƒ¼7©:?Æ5èDL‹?í•9î8W_¿âãeூº¿Ð`LpñÛ¿ÝÓ]ÀOâ¿æßÛÒú
xUNASNone3FGL J1155.3-1112?ïúHѳ™þ??aF9–	?Fܹà÷Hd??aF9–	?ïì3vòG'?c«'¿Y¢?c̈ò;øþ?c«'¿Y¢?ïÒjæ¨Àÿ?u´hu\êç?vʌ¬Ol?u´hu\êç?ïݔš6Ò?TþXáDµ[?q5³ÒS?TþXáDµ[?ïúQöþà¬?FT°är8g?F¸$–,½¦?FT°är8g?ï·¤>¿Ð?Œ{D! —B?'ð…¯D
?Œ{D! —B?ïâõ¹]·Ê?v±¼öòð?m
F…k~o?v±¼öòð?kný?y¤C©;Û?ŠÕå'Ì°?y¤C©;ÛAGN4FGL J1157.7-6327¿¸Þ8P›§P¿óQÚ7ïZ–À8ô".E©À:•,oʓ7@>8?6¡¨@ÏKaþ!Ù?ɔš×1T·?֊MÌ;­U@áã!¢ç÷@÷ÚE±:?ìÚã{dû,?½ê2S¿ç×Tz«—É¿ëb)ösD¿îBýûÈä¿ðUNASNone?âçV™r`?Ð+ä==	?ÛÜ1RÍ@?Ð+ä==	?Ö®1£ˆ}4?Êg{Ëc§V?ä¨ç.;Áf?Êg{Ëc§V?ã€úË7Ì?²Ê)'@Q ?Øÿð
ig?²Ê)'@Q ?à%·d…»–?²ýšÓÝ6?ß´'6ôˆÓ?²ýšÓÝ6?ÔÖá2àR?Ñ…ŒÏå9?唏fÖø?Ñ…ŒÏå9? ng¤šw½?­õ[+1Í|?îù…ÑÕd?­õ[+1Í|?ÈÎR¡–q?²ñ™;ÏÌ?éÌk{ךd?²ñ™;ÏÌ?™­()°K¹?‡yOQk?ï2–¾{ƒã?‡yOQkMIXED4FGL J1158.8-1430?îº;h@G:‰ãC0×À;ÊNmK]À<}ª?K@!ˆ~7éPf?þ±ÞŸ]'ù?ÁŸ¡EŠx¿¿®å;µg?ïèÞ%d¾?í·«^×À‹?Ô}ÖÅt÷?|¹H­æ$.¿èqԞ}Y¿æ(ŠbÄñ¿Ê"Î×Ë®¿…Ôª'¹{aUNASNone?ïÕAqÔ'?°ðLXÉå?u_G! c`?°ðLXÉå?ïež¼‡ôð?œ!ºÏo?"L(rpýò?œ!ºÏo?ïÁu°}®#?óÔߧF?E'Ã8²x?óÔߧF?ï¨5ùǵ?s%˜&*5?…ò¾~vµ?s%˜&*5?ïùþ'7¹f?R'1>ßf?Höß®¥D?R'1>ßf?ëØg¾2ß?ÆÝ	ÀÖ[?Ãðža4…?ÆÝ	ÀÖ[?ï¼sUN?"#
@óIÀ?€ã`"ž?"#
@óIÀ?ëöqµ¾­?²%
áNqÐ?À&9)K³?²%
áNqÐAGN4FGL J1202.9+5818¿ï™ä[ùj@L×z_A®÷À;'bþÒÙVÀ<½·ªü˜l@(¶o\@HÿÚpú?ÄÙ»G¿1Y¿›Ï(¿`n?Ñs×þ")ñ@òà¦ÉX?ïøÀÛýÂ8¿ãÚ¥hõX¿éfòH‡X¿îQ•	ÖC?äp@¥½£¿êÚýç÷ËUNASNone?﵊æDåZ?²ZËÂ?'F_¨aª?²ZËÂ?ï÷õؽNˆ?QÅujè7¬?PN6I?QÅujè7¬?ïÇ_RJû|?€¹²¢Û?|PVº5î<?€¹²¢Û?ïÿz®
ْ?ÿÏÞÀ?ªF˜8F´?ÿÏÞÀ?ïú*'ó»?UnË;*?GU³ºr€?UnË;*?ïÞ¾÷CE?rQÜéÿ?p "nµýj?rQÜéÿ?ïTÅõv?‰ùâgeUI?ˆªþQò>‹?‰ùâgeUI?ïù—RŽåƒ?JbäÓoµø?I¢¶ÓþEì?JbäÓoµøAGN4FGL J1203.4-6145¿Ùˆ#:Ò*?âé*ÁI¶ØÀ9ƒ×Ð6
ÙÀ:Ñ;§uû/@àúãe@Y~™cõ?ËPk'kSá?Ú=Z¾è]¢@½C^#¡Æ@VÒõÜ?ïÿ9œf¿äӟNå@¿åuWСm£¿êUŒáû2¿ïÿÕ%t.¿íýØ=CWnUNASNone?ãz
w·Ç'?Ìé9ªp¬e?Ùåpü?Ìé9ªp¬e?Ùf­þdÅ?ÊÐiSDk?ãL©óMž?ÊÐiSDk?å{omÝ9h?³7ÿ®Ù;?Õ	!$E1?³7ÿ®Ù;?ã֗y-éG?²ºà´\ÔÇ?ØRÑ
¤-q?²ºà´\ÔÇ?ÓjˆPð?Æ؃d"?æJ»±W·ˆ?Æ؃d"?Ÿ?Ùl"ê
?¬»ÓQ"ÿ?ï4ēÿ?¬»ÓQ"ÿ?ȾWÃO9h?±8¸Œ±¦A?éÐj,1¦?±8¸Œ±¦A?§_ñiOª?"W‹dõ
Ž?îŠéxÃÐ?"W‹dõ
ŽMIXED4FGL J1203.5-1748¿ÖXþ¢'x@E˺Ü	€²À:d&°mñÀ<gÍ0ŸÚü@ý}}":7@…±ã<zÛ?Ȩ|¶^÷1?Ðӛ=]®‡@{ÜpêN@jlU\(¿î³zK¹?ïzV¨ƒAi¿âÍg'ߐõ¿âÁa~õÿK¿î'(]í¿ïÿ•AED®UNASNone3FGL J1203.9-1745?ïgéÜ?–ìÚFMX?"Üÿ}?–ìÚFMX?î"ÓË•?¦1ÍZûÊ?¦¾'ÂsŸ¸?¦1ÍZûÊ?îAˆë˜â1?˜S£Æ7??«çqB&Yö?˜S£Æ7??íÎ[PÄϹ?''VH$öž?±%ykŽµ?''VH$öž?íB¤é¥X?²–"zôI?µêØ·4á¾?²–"zôI?é±sV,§?Ǽ"£¡â?É:2§ƒMc?Ǽ"£¡â?èÓí­ö?³"цQ?Ì°K±H%Í?³"цQ?äâÑùÝQ)?º¢Ì7ƒ	?Ö:\E]­?º¢Ì7ƒ	AGN4FGL J1203.5-5745?ÔR"¢jÑ@"!Š"CÀ:˜Ž:À;Ö©n"óJ@aÎQ1@ ;êŠ?ÛÓuþ‰Þ;?àÈðÔéÑÀ@YcˆÕý?ü%͌Fµ?ïøÕ~Í"?Þ0×Cÿ¿çcvÇÝyÿé·R²T{'¿ïýðƧÞ?ïâÆ3U—âUNASNone?í°³­}7t?¸Õ'ð|?²zb"ò+[?¸Õ'ð|?ßËÂÍ*ÑÌ?ξ2
TF?à™j—?ξ2
TF?슨¡/¡?¤*ï/ڎ?¿ªºö'ö?¤*ï/ڎ?æ{@+æ'?³¿ô*Ârí?Ó	ݨ3³?³¿ô*Ârí?åûIMœu?ÌÉöo€Û?Ô	meøÇ?ÌÉöo€Û?¢oüÄ	¥]?°M$òü×ï?îÙ3£èÊ?°M$òü×ï?àȇ‹Ø™g?¹ÐË'8ܞ?ÞnðèNÍ1?¹ÐË'8ܞ?®'ö&(ý?žÍљ5&Æ?¸üÐ?žÍљ5&ÆMIXED4FGL J1203.9-6242¿ã
ôu濛¿Õ£òfa´À7럓®žÀ:ƒÝ ×æÜ@åÈøן@lû@}ž'?«uPºÃú?Õå@Ìxé÷@(0ítA@ÁÊqRӍ?îc'ŸÐ¿Õ†šË'¿áW›ÝÁ'°¿æHiü¿ìòFñ'¿ïÿúVrÓ\UNASNone3FGL J1203.9-6243?O8W_݋Y?P'³½ÄÆ?ïø1êU@F?P'³½ÄÆ?¬ÉnÀÊWt?¦^8,l÷?î3ióZ‰?¦^8,l÷?"±QNÚ·$?'JÝЩpê?ïZuu‰*G?'JÝЩpê?}¤]S€x;?rÏÒðæ",?ïÄ·E9?rÏÒðæ",?K"ò'³–M?Hm]ã??ïùˆíò?Hm]ã??D'~C?€ö"λ¾?ïÁvܝÃ?€ö"λ¾?"³w'èãI?sýãòJè?ï­2!ݗÃ?sýãòJè?#%a¾Û`?·O|ßã?ïÿ¿s¦sz?·O|ßãPSR4FGL J1204.3-6111¿Ù'©ŠtÛ?ò¬š'^ÛÀ9Ù¨g'¶QÀ;(Ag©]@úhýoî@悀x`?ԐY—Œy?àœ<ÁÒGá@
ƒn´é?þÀøãÖÿ?ß{ûú?ƒ`MŒiŸ¿çÒ(ÁÀ)P¿í[ˆêዿè.]@L÷*¿ïÿÖDDÓoUNASNone?âûÑ?ÚH} «àÞ?ÛùÃÔ]û?ÚH} «àÞ?ÖÑ	t•J¢?Ê(¼ÈÙß?ä—{EµZ¯?Ê(¼ÈÙß?èƒÍaó,?²`pr{??ÍðÊx3ÃQ?²`pr{??ãtŠ'"3B?µ'ËÒо?Ùêúי|?µ'ËÒо?Ý&]€þ\?Ò­§C·v
?álÑ?€Ò?Ò­§C·v
?˜<¬ˆÓ†w?¤‡ì'{™?ï>›æì?¤‡ì'{™?ØL¼¾?¼Uñy)Œ–?ãÙ¡óôó¡?¼Uñy)Œ–?¤ßå½»`4?šgÊ»Šš?Í?šgÊ»ŠšMIXED4FGL J1204.5-5032?ïó±'eí½@'Eík¨Å‡À:]4=õ.À<ˆ໗@æKùӖ@œ…Ý$3?Æ4¸Œ£è?èΙ«7@ Ù#¯2@cLÝ(d£?ïìQ'(¹³¿Ô–)ÂÇt¿ÉôuˆBYA¿è_[5z`¿ïùΝ²X¿ïí¦–Ø:UNASNone?´òQP0˜D?½ÃÓSb?íaµÕÂó8?½ÃÓSb?øêPÚý¬?ºKK©‡ßn?ëÅkÉ@•?ºKK©‡ßn?Ó´ ˆá~?±œ×®hÒ?æ%ﻏ7Á?±œ×®hÒ?ÓH"
í?¬õüAÀ¥Þ?ætÛ¶8zŠ?¬õüAÀ¥Þ?˜¥¯[à–ý?¸»h©ë)?ï:҅.¹¸?¸»h©ë)?'r¿RJV?"ð+oÇ"?ïlj¤§?"ð+oÇ"?¬+D? ïyâÿp?î>ÿÛ
0? ïyâÿp?šHÜ+©?ï?ƒ´"1×?ï-¹¢¶?ƒ´"1×PSR4FGL J1205.1-5951¿ÐJ¼O.Äí@ü¢¢&0À:1š‰ƒ¡áÀ;œz'
‹@°†ðõv@…õ'^éš?Ç7ªÉlÆ?ª3¤r:¯ÿ?漺Ñ!Æ#@‹9&A³¿âîO~mnB?ïøYþyC¿èˆV{6Ø¿â­RH¢0A¿í/†ÖHv'?Òja}ss?UNASNone?ïØ1©_#@?t}'vÀsÊ?sç+Gd?t}'vÀsÊ?ï½í
´ôi?‹
Á‰~—«?€"¼ŸÑi±?‹
Á‰~—«?ï‰é<2û?'Cåéñy>?.ÂßXؙ?'Cåéñy>?ïɃËõ?dÑíÀÎ9?{¶¥´&-?dÑíÀÎ9?ï<€Åû?˜¨{ãþW?˜oç[¨Ï?˜¨{ãþW?íPG÷C š?¿Ú}0ú–+?µ}ÀFTî²?¿Ú}0ú–+?írk;|É?¤ÄÌx>*?´l¦#C:¸?¤ÄÌx>*?î[ŒÑ?Ÿy]:Íï'?®.šFb›ô?Ÿy]:Íï'AGN4FGL J1206.8-6038c¿âF`‰O
?ü4xã@¬˜À9ÌAƆbÀ;%ÿÜđ•@Êæ¼7(`@.ùèŽÊ?ÐÒíÌw?Ï`Š™ÌoZ@¹5v'\@qæOx?ì¿-b
翱ɫ/C9'¿èöĝSb~¿ä¶‡æ鯿ð?ﶞaUNASNone?ïrª(Ç?"üoI0lý?'¬J·Žk ?"üoI0lý?êñו ?Âó9?‰$N?ÅÀ8¡©ã?Âó9?‰$N?íW»Ab¾? äü€"úÅ?µB%÷šÝ? äü€"úÅ?í%FÅ{
¬? ™"K:ƒ?¶ÕÉÔ''Ÿ? ™"K:ƒ?í¯ÈNýƒ?´%ßÈÞóÄ?²‡¡¿?áæ?´%ßÈÞóÄ?ɨ]¨bñM?ÌVHÐÃX?é•è•çC­?ÌVHÐÃX?àn-`4H?ºnò¦ü?ß#¥×?—p?ºnò¦ü?Ñ/Ú*â?º&žÐ:@?çhtÿê?º&žÐ:@ MIXED4FGL J1206.8-5836¿ÐiÈCƒÀó@…`&±EÀ:»™ž¢À;ØA'è|V@ê×yÎù@I¥ë·sŸ?ÕÙ*ÞÐÛO?é›ü_âhÀ@¥º9LR@YCNa?ïôáÙú2¿ß1É~X¿å~®@ð‹¿ï!ÃÔֆŠ¿Õ=ŠÅ@fx¿ïþÿðÇôUNASNone?îÓ°€)ÊÃ?"=åœZ?¢Ä÷úϞÌ?"=åœZ?ì'2>"?¾)ë¡NCÛ?»nk¦ó?¾)ë¡NCÛ?íbV¯9>?¡üÍæ:L¦?´íJ‡í݄?¡üÍæ:L¦?îáõ1ÞA?Œ‰Ízšñv?¡à¦üâò?Œ‰Ízšñv?îS7©©K?µ˜Â¡S6?ªÌ…aû³ð?µ˜Â¡S6?Ҫʕ I]?Ðӄf×z{?檚µoÛR?Ðӄf×z{?ç3y8È?¶I¾:ì"?љáÒp?¶I¾:ì"?ã;§Á%ò?Äסì=DH?و±æ}´?Äסì=DH	MIXED4FGL J1207.4-1840?큮¶Ó;@E}NÂò®À;@Ë]a'À<˜Šï²ªã@'¢ivç?þ¦êjl…d?ÓÒÆáÑ@Ð?ВôÏJU?ýkؖ.«@(*…È¿ïüþX`f?ïü1©Æ7‡¿ÙÓåŐ¿æ{°&äp¿ÙÿÛíÒ¿ïÿõEq#UNASNone?ïýô¥-÷_?$ŸŒÈ¹þ?0ZÖì?$ŸŒÈ¹þ?ïïÿK}?`xñãB")?`äé8'=?`xñãB")?ïÔþô߇Ý?mäêY?u€…¨IUw?mäêY?ïó(´²­D?CMYü‰|?Y®–âV©?CMYü‰|?ïý¶ƒN?/ÿÔI+¯â?2KåÒV	?/ÿÔI+¯â?ï·þBªcZ?ýÙfìÜ?'oamËc?ýÙfìÜ?ïªâ‹ c?ƒ5hô¶wØ?…G{¤L?ƒ5hô¶wØ?￶I†9s?rIé E™ã?€mŸy…8?rIé E™ãAGN4FGL J1207.4-4536?í͂ù*_
@0"süPHÀ:tŽ·¾GÏÀ<}MPëªÞ@`Tßd?ÿ<¼æ¥¼?Æt~A¤e%?á7^3'þ@#¥ ¶Xí?ñš0Å´Ö?ïÛi³"Ü¿Úï
Kšˆ¿ÎÊ.·Îbú¿æŒ x°ì¿ïÿ
A1"¸?ÊĦ}ìUNASNone3FGL J1207.6-4537?ދ©ÂÜD?ϦKpc6Ó?àº+w'Þ?ϦKpc6Ó?ȟ÷!	:?Á^
$^a¾?éØ7½±|?Á^
$^a¾?×åKu썪?±ö~•˶?ä
ZE	¹+?±ö~•˶?К¿î[׆?¯ò0èãÖ??ç² Ò=?¯ò0èãÖ??©[œQ•˜?ºÂNLFÞ?îjF:ª~w?ºÂNLFÞ?›Tr0´¥? îq@ºf?ï%\nH›? îq@ºf?°íê*øôj?Ÿ»Cqö¶?íâBºå™¢?Ÿ»Cqö¶?'ÝO´ 
?ƒPc•o?ïq‡YX¿?ƒPc•oPSR4FGL J1207.9-6443c¿ï¬ÍKDCÀþ}~°àÀ9ÃÚ#Íd¢À;@+ôzÀ@ü¦¬| @ÍG`ç¡d?ǎ¾^9ò?Û`–ƒ9°Ñ@"yJ@«"6‹­H?ï#BÅwmö¿Ý}M¾NÚ¯¿á~@Ï~¿åOãm"BJ¿ïÿþÞ÷?íkP`j£ãUNASNone?ål/TÆÄ?ÉgôâPÓ¾?Õ'¡VsÌx?ÉgôâPÓ¾?èl]*mÄ?ÇËM¯ ?ÎN‹W¦Hî?ÇËM¯ ?åé¨rô?²eÚE?Õð,¯È?²eÚE?ìÇé°±ˆ?¡Àޅp'›?¹À²|s¼?¡Àޅp'›?Òe»Wi¸?Ê3Yó?æÍ"uÔK$?Ê3Yó?¼né€?Ã^Œ€U•?ì}Ò>âÐ?Ã^Œ€U•?»Y0¢#Ï?§*қÑ?ì"Ù뻜Æ?§*қÑ?Ñíb"Rf?¸Š~$.nº?ç	@NµÖÍ?¸Š~$.nº$MIXED4FGL J1208.0-6900¿êŒ"+ëmÀÖ¢?ZˆãÀ9ú¦wÎm·À<åaïa@*AþR*ð@âÛ,!?À9­å×?×ù%ò-/@ÅJ]ò#ž?ü«?#VqQ¿í¯/˜sÿ¬?ßÑ%ʟ¿à¬ÅZèƒâ¿å'¹ñ·é¿ïÿí¡Ā?é7"^6UNASNone3FGL J1208.0-6901?ÙÈeólÒ?Ïâ8"‰#?ãÍ|†I—?Ïâ8"‰#?Ý|ò
ý?Í6"T´{?áA†Àyt?Í6"T´{?Ø\`R
Ã?³óúta?ãÑÏÖõù?³óúta?èN¹ì QÅ?±_^"̽ñ?ÎÅM~¸î?±_^"̽ñ?¦|OGã?¯<ÑS°†d?î˜>«†ò?¯<ÑS°†d?¬Yq»©ñ?´Ù.ÞNzC?î:n¹?!?´Ù.ÞNzC?«`ÜI®L?eR)ð?îIò?")Ì?eR)ð?¼¼G:ôj?¬I_D‰?ìhw¡r½?¬I_D‰MIXED4FGL J1208.2+1158¿ïó%§Œÿá@QñŠ '§À;<n—OßÀ<·;÷ýÒÿ@¡è:@g¸Õ¥¹?л›nÛÖ?ÃsÞt$?óèÚI@E¹F]1‰?³õ¯o烿Þà#`"*¿æîÉp!¿Ó(ËÑ$J¿ïÿÿ" 5•?ïÿú@ùDzUNASNone?ïûæön±¹?BӅ;ªú?@d%7×»ž?BӅ;ªú?ïóÙ¦¤ïä?^6\êXý?XL²kè¨k?^6\êXý?ï~wÂ.c?Œ±$¿kÔÿ?>J—?Œ±$¿kÔÿ?ïö¥U[ôj?@lÔì°ù?RµU‡OûÐ?@lÔì°ù?ïúœÄxV?GncX·Ä?EŒï/)æ'?GncX·Ä?ïÅ­eB=×?†æd8éÊl?})MS2h›?†æd8éÊl?ïƒ\ã¨'ô?Ž…»µ0™?(ÇÕ:ê?Ž…»µ0™?ïÉañÆ]?n*Ÿµh?{Onn%­?n*ŸµhAGN4FGL J1208.5-5512?¶¯'«ù@­\œ¹À:Š÷mŠGÀ<'8Yã¡%@×XìÖ-@¥Ò! c¸?О#y+æ?Ö½±[­$ç@P—\¨wƒ?þýîþOü˜?îç%pÔ)¿ßg"ÄËL¿åìÏ¡"c¿ÞB(.rý¿îõõO¢Õ'¿ï#'ŸÐ€UNASNone?ïy¥Mø?†Â'P}¦?Ë^"‰/+?†Â'P}¦?íy¦4³?²ÏL)GxÅ?´7ÿH¨˜ï?²ÏL)GxÅ?î'R{<?•˜Œ[öÿ?§ßNjØLC?•˜Œ[öÿ?î#ËGwÊ?†y#ë26¶?®-ÃM@Q^?†y#ë26¶?î~"D?¥ÈSZ3ìÛ?®Ö(K6¿?¥ÈSZ3ìÛ?à@	'k?ÐÎOò?ßçí˱*?ÐÎOò?êGòíìO?°km,l*?Æà7ÐHNÆ?°km,l*?å;7ïí?­A»‡ç%Ð?ՉâŐ '?­A»‡ç%ÐAGN4FGL J1209.2-7635?Ù:Vn‡Ù9À+×ÆÚD""À:Ûe¿wy´À<1"óg°@5°!›[;@›Y<²7ö?˚¸Å-ò?­&û#9t?㑺ýíV/@C%<û^?ì³vð!e«¿ÂdŽŠqÞj¿à&}­ªÈ–¿äÜ`ô6ž"¿×€´ÿÄ¿ïθʷH×UNASNone?ïûiæÐ?:t_˜xè?B[˜e¤G£?:t_˜xè?ïìy®Ô?l'‹·?cä†%î,?l'‹·?ïÑ*äs÷7?wi'$¡¾?wjÞÁ"$?wi'$¡¾?ïïô»íñ$?DDlÍ‡?`CþÑ"?DDlÍ‡?ïòà÷ôe:?YÆÀvƒ¼!?Z>Ê>MQ?YÆÀvƒ¼!?ï¼IMÏ?"]ý§Íˆ?€í¼w
T\?"]ý§Íˆ?¤uÑÏ?Š²'Nº?ŒVÖìÚ`?Š²'Nº?ï"Qžƒ8Y?zϋ—ó7?‹+˜i€½¤?zϋ—ó7AGN4FGL J1209.4-6421c¿ïù™ƒ–šX¿ý"€Û\²ˆÀ9"$¼wêóÀ:÷bLLà@ÏrÅz%@#_=}9?ѱœÃ,?Æì¿o?ÿˆÑ•‰i¡?þ\3!•{þ¿ïJAl±Ú?ïõºAYç}¿äÔ6þÄÁ'¿ëôÿñ½G¿éÁ2?B`"¿Ùúc
UNASNone?pCÚuW?PÊkö'¢?€›îøŒ"\?PÊkö'¢?í¶ÿvÿL?³fµì·6?²HFMÑ¡?³fµì·6?íL{&kz?£N_-n?µœ'þ̤3?£N_-n?íú‡¸"?•4j²ÿ°Ë?°+Â?Üã?•4j²ÿ°Ë?é!Ñ¿ƒ?Æà
AL|?ËÂx¹ò?Æà
AL|?âr«Í½|g?Ô"Ŭ
ú?Û¨d…3?Ô"Ŭ
ú?â	=ý´?¼ « e?ÛÙíã"˜?¼ « e?Úºï§dªÇ?ÀÊÇ]î"?⢈,Mª?ÀÊÇ]î"8MIXED4FGL J1210.1+3241¿ì³ç^ڒ@SÞ\å´$_À;ÅÚ(ÕâÀ<é(kYn@!\tWë¤S?ûYê¦Òg?Ù>4ƒ•KV?¯ô¾®Q¶?Þý-<ÏN?ýíôOG»Ö¿ïþh›Œ¹?ïúµÞs¾>¿â¿Àʶ¿ïsøö ƒ?î0?)á{¿ïÿ¸GʐUNASNone?ïÿMfvgÌ?&uäÒâÄf?S0¼»Y?&uäÒâÄf?ïömº?YW¯‹Àµ?S×$&>oà?YW¯‹Àµ?p.;R?‰ß†ZD?Ycê"W ?‰ß†ZD?ïþ£ÚUˆ?"ÚÃéwõÿ?%Â^òwÄ?"ÚÃéwõÿ?ïþô‡v?.ˆFN‡?'à¶.!xu?.ˆFN‡?ïÕå%oas?|I-œ¨e?u
mcÌ&`?|I-œ¨e?ï;–;}?"¬þÛz«?˜0·Èo?"¬þÛz«?ïò¥«íüj?b!جÑÈ?Z´§×ìë?b!جÑÈAGN4FGL J1210.4-6250¿ïv·FJ3¢¿ÕmÒÁXzjÀ9XsHÍÀ:še"¯O@¦—Ìdòô@ø¶zzða?Ð"Ág	?ëøìæGÈ@s@ªÀ3?ùU®ˆ>(¿ê w~瑟?¼ÚÇ·9<¸¿ÜK¹ý<VH¿îz̺XV¿àŸÑß[E¿ïÿ2Ȫ(UNASNone?áÇÒ^~‡è?Ó®Zƒ%±7?Üp[Cð1?Ó®Zƒ%±7?ÀŠ'\v‰°?¸;¶Í\?ëÝv(â]"?¸;¶Í\?ß±goêl?³Ì'•¶'€?à'LH
¹J?³Ì'•¶'€?Áü0£Èó?ª†Âšwm¨?ë€ó×
ÿƒ?ª†Âšwm¨?È'w"4z±?Ì#®õ)G?éö"2áT?Ì#®õ)G?…£^@1†P?‡·ECY…¨?ï©r‡(u7?‡·ECY…¨?׎]GÑ_?½Vb¢·z€?ä8Ñ\qÐ?½Vb¢·z€?bÁ*¬Æ,?`PfES!?ïí>rè'
?`PfES!MIXED4FGL J1210.4-6100c¿ì™Ïª«Bl?÷|…Ý$2åÀ:@ù¬(èWÀ;igI»4õ@ H.}ÁÌ¿@‡åÝ?
Ø?˪µJÐë?²ór}öÑ?íá8ÿûÎB@VÃÉBÿ"¿ëü'§:?ác¢1пÚ*{žÜÏy¿å¬vJßø#¿èÁ‹ ²'¿åWÃ Ô ~UNASNone?ïö»Y?h'í–"…ó?Rzz~N*?h'í–"…ó?ïØùë,Î?€{ke_?sƒ
Q‹º"?€{ke_?ïy'wFL?Œb Ò¬u?Ï¾‹ïÌ|?Œb Ò¬u?ïé
†p6?RMûÞ¬J?fõyèoÐ?RMûÞ¬J?ïÅzI¶ò	?"9=^"\á?}BÛI+«?"9=^"\á?î–a†,ÕK?³ï±%{?¦™çœVÄO?³ï±%{?íÉý5å?¦kÔÃÉë\?±°Oüg?¦kÔÃÉë\?ïR±ÌÕ?ˆí·ZÇÞ?•©ÆxÏép?ˆí·ZÇÞ8AGN4FGL J1210.7-6005c¿êÆfäx@	1*À:n+ë†ÌÀ;k*þ±K@ 	ÃÑ%¡û@të<#œ½?Õ[H{úù?ÆLCe'Š?÷&q3I¨@$lÆÒ¸¿ïøcß"Í?ïÿvmD¦ù¿çQÁÚM¿æÂ:½k/ú¿áFmlêäæ¿çp$ sRˆUNASNone?ïñoÎ*V?k}¾R¹=?\Å `룸?k}¾R¹=?ï«ÜçÐ?$É޼֎?…Æ.?[õ?$É޼֎?ï4¢•ÛbÖ?"u]Tbæ|?™k­BÛ×3?"u]Tbæ|?ïÛ˳ž?a}Ý 4‹?rqš_YÝ7?a}Ý 4‹?ïÀ†?«¢íj¦?ˆx1'8?«¢íj¦?ìvßׅQR?£3#'?¼ICÕup?£3#'?ì:£{+?±5͇ÖÐ;?¿æ*ä&¨?±5͇ÖÐ;?í²üÒ#"ð?©5𮧓?²hm/"?©5𮧓8AGN4FGL J1213.1-5957¿î•@…šøÙ@ø¨ó©°À:Ç"hà"À;²þ¾·`T@Wÿ¡`bk@ށËFºÏ?Հ"ûOA1?ãÇkcü(Û@F{åS¬?üü‰Ñ$ H¿ï÷fÁ1
?ïúõ—k¿á£8I©"¿ä\«!Vfê¿ïþæŜVã¿ßëXZ4)UNASNone?àL1²]={?Êü?Üûø?ßgœ›E…	?Êü?Üûø?Ö%à,ƒŸ:?Ê/'ÐãÃð?äíé¾0c?Ê/'ÐãÃð?柟́`U?²(A
ãé?ÒÁLd÷?V?²(A
ãé?äÊù8¼?±L³"ÉÜí?×j
àˆ?±L³"ÉÜí?Ã4¹+kyÝ?ÁÛA"·ò?ë2ѵ%!‰?ÁÛA"·ò?˜ìä(åР?£ó)à|–¤?ï8˜ÞïË;?£ó)à|–¤?ÃÏ¡ô!­?²`øª€"?ë'þw•?²`øª€"?®v3ïã֓?š8Ë}¶Fö?îœÁ8¼V?š8Ë}¶FöMIXED4FGL J1213.9-4416?ê·¿T>E¶@2b€'،À9ÿ'xë¤(À;÷%=§*|@c®%AÙ@[¹™ê!q?¼b?PÍÎ?ÍhŽŸ? Õ@m.¼«íY@aBŽ?ï»|þX`?ğÚ{aU¿åZ³uòW¿ãû}å3 ¿ëmª]6;ü¿îlЮÝ*UNASNone3FGL J1213.9-4412?çf¼/Vì?Ĭkß³?™?Ñ3ȇ¡R(?Ĭkß³?™?ârWÍé¤Á?Èù¨Q\,ë?ÛPd,¶~?Èù¨Q\,ë?ëw°3á?¨U4u3¥ø?Â!?¯‡0z?¨U4u3¥ø?éSéœM?£>PdФ?Ë®³˜YŽÎ?£>PdФ?µSMÔÐû{?²ûÚg¦=¨?íU–E.æÑ?²ûÚg¦=¨?¹¹[FpÔ?Á´/I;)Ä?ìÏÈԉsv?Á´/I;)Ä?ÑɚWŒó?·®Zd2?ç2Ôq9‡?·®Zd2?È£tœÍ?§‰EÌÒ?é×>"Øû?§‰EÌÒMIXED4FGL J1214.5-2318¿ï·Žì0Y(@Cc‰!S7À:ӕÄ"`À<o]2K­@\Ž´
c@?ýהÁÄO?Ô(ªÄbC?Ñ.…dˆñ?ÿÏ'T·@øSK+¢p¿ÕC	ËÜ?ê#X)ŒÁD¿Ó¬¡«¶Ó¿ÞӎóMj¿äøSδ-š¿ïÿ7¸Óñ"UNASNone3FGL J1214.4-2315?ïýpH'jü?1("à2
æ?4}»‰>x_?1("à2
æ?ïðü¢ñ?_·s¼?^ÄýºžT?_·s¼?ïÛHÈñ í?pJÔ}p?r[›¡L'Œ?pJÔ}p?ïê¢u¶:?GÕí …ù?e]Š6‡ þ?GÕí …ù?ïþ%žu?)Ûׅ¿‹Ï?/
¨þ!ôp?)Ûׅ¿‹Ï?ïÉ¥¹@?‰JÇ
@"?~~»	?‰JÇ
@"?ïÏ´'Ì?~ZýÈ/hª?x%À=y0Ž?~ZýÈ/hª?ï¼·}'¢?k_¥ð¨"?€Ò Åܑf?k_¥ð¨"AGN4FGL J1214.7-5858¿ï
Š¯Æו@'Ä$#À9¦`;©ú:À;kT/,=v@ÛÌ{O,@-¦¿
"?ÈïcЉð¯?ÁÏ+KÞ$ä?þ<xVRòì@•€ZXf?ËM¹Ü°¹¿½håq´MO¿é^´ás¢å¿æ1neZοïÿs³VB?ï¾h…ûW$UNASNone?ïÚ³‰s z?u»KCjûÜ?r¦;)S
ì?u»KCjûÜ?îÊÚÀfž+?©# ¯a§Ç?£RSýá L?©# ¯a§Ç?î¿si?oé?"<´×óþ?¤ÉpT"o?"<´×óþ?ï0CUŒœ?'|É Ér?™ýWŽo4?'|É Ér?ëÄy
ªZ?'ú'Bñ?ÐîÉV˜?'ú'Bñ?ã£ñ{Ä?ѹóÅù¸­?Ùæ¸	Èx?ѹóÅù¸­?ç&¬iLl7?¼¦¤".?Ѳ§-g'"?¼¦¤".?æ.º3~Bâ?ºsbÇõ?Ó¢‹™z<?ºsbÇõAGN4FGL J1216.2+0537¿ìeC'­Å@P»>-b9À;}JØkf€À<¶]ŠÒS@ R"²,?ÿ«cÆxö?ÕV¶JªH?Σ€ùÊ?êžwïû¥þ@	&'=TŸ??¯®Ï¶·Å?¨Ã=ë¨¿ÔÝç®Ðc¿åÕuþ3÷ÿ¿Ü4ÄØ·'¿ìÐ=ÊeêUNASNone?ïý-—Å?2Wكž}?6—Ub"Ò¡?2Wكž}?ïô»2	M?\ø…RÞËÝ?V‰›¨E6Ÿ?\ø…RÞËÝ?ïÛH9™m"?k"þÈŸÛ?r[ã3ù"2?k"þÈŸÛ?ïû.'…Eq?+ááŠoO?CE¹r"¹	?+ááŠoO?ïþklyi½?&°&z®ÿ?)I:`÷·õ?&°&z®ÿ?ïË·™½^x?"G€í…9õ?z$3OÕ?"G€í…9õ?ïÔv¼lO?€²Gé`DÑ?~5ęŠÈ¡?€²Gé`DÑ?ïïæiK7?Q`ÚByŸÆ?`ÿ²1¨à?Q`ÚByŸÆAGN4FGL J1216.2-0600¿ËÈ-ß>òã@Kå2µ^ñþÀ9ÈÏuôxãÀ<,νgÔû@¸™nÑnó@—¯ê=öÜ?¸óÓÌÆAÃ?½Té;mie?þ±Á
{é…@D,²™Æ¿àsûz_B¿âž.>VÒ˿蟦=ìʙ¿âtŒ>'6ú¿ï¿¸Så¿ðUNASNone3FGL J1216.6-0557?ïÛ¾˜Û{?nZœó‡?r ö,³
†?nZœó‡?ï²9ñQx?ˆå/ÞÙ®v?ƒq½ÊâÐ?ˆå/ÞÙ®v?ï7Õ¬šRQ?'ÂUü?™JuL»Î?'ÂUü?ï/Û©Ðr?ƒ<êÝ%)ñ?šŠÞ}¿Â?ƒ<êÝ%)ñ?ï\úüNßP?2öJÀ/À?"` tlH?2öJÀ/À?îZ@6b"ñ?²j‡|±b€?ª[ü™ÝÐð?²j‡|±b€?î[ùŒH?¢*Ô[_ÂË?¯:N±C"w?¢*Ô[_ÂË?ê;ú'>?±÷JJû­?Çø·¥?±÷JJû­AGN4FGL J1216.2-1550¿²TBô«7@G5ü;OaÀ;W%­AíÀ<šÖvš@ JB¾@
¤‡3f?Оi¢…üY?®®£Áæ"Ê?߸©)Y•ž?÷¼"*F¦?æáJ2S9¿ÕãvÇÝyÿԒ/BêÊ¿çÚ\FQô?—˜×…k¿ïðÃhŸýUNASNone?ï÷z˜ú°?…Oþ?Q̤ÏPâ?…Oþ?ïäIåšÔ?t–ØxïVm?k¶`+†?t–ØxïVm?ïÍՄg"u?v¹ÊAt§?y=´Øm¢?v¹ÊAt§?ïí¤†0?Nÿ9t«E?b[yŒ¬ Û?Nÿ9t«E?ïú½d¾µL?G'ñèøO?E
m¡Ù$?G'ñèøO?-MÒ?•îߟ¡ì0?‹ø~û_g?•îߟ¡ì0?ï¹hLŠÑ?ƒLF·?ãî?¥ù³—Ë?ƒLF·?ãî?ï~၇ "?""– îV?#ÏÕû%¤?""– îVAGN4FGL J1216.4-1358?ÚHqL¸.I@HŸU›=À;&:Wê£À<…AøDJ@ [&¤«@5ºÚ\‰?Å}®ˆ*Ü¿|8ù" Ðý?¶POx¹$N@<€;¤›Ö¿ï·1Å?ï îؐO?ÎH»…§ŸA¿çviéпïø£NNB?ï인KhUNASNone?ïüÒ'4ú?5¨·ü.a·?9oa³‹tž?5¨·ü.a·?ïôóŽO?ZÞ1ña#(?WÎVÔÕ/?ZÞ1ña#(?ïR_CÉó?ŒÜ°À]ÅÜ?•´zö]˜?ŒÜ°À]ÅÜ?ïø3lLJ?AQi³6{T?MÃ1Óï¤;?AQi³6{T?ïùØEü¹z?Kp]Bç!Ð?HžèÚ)/&?Kp]Bç!Ð?ïͦ!‡(?~X5îpØÓ?y,ÿé×Õ?~X5îpØÓ?ïauD¥?'SbÅËei?"Ü'X0u?'SbÅËei?ïêƊ"lY?`*Gáœç?e9uŠÐ6ç?`*GáœçAGN4FGL J1216.8-5955¿ïžB®®Ý+@>ØÓkLÀ9bsýþžÀ;%‡\€3—@/ÛåÄj@¾S<½öp?À愙WT{?Ï{£ºY؎@9[Ývh<@èÀr×
?áRá"öW¿áôÁÞ\A¿è9Xç!â©¿æZÙ㐿îgñ`ªåœ¿ïåaHÌ"UNASNone?æꥶï|?Ä$?‰q?Óè*´'!?Ä$?‰q?Ý­®GRN?Ê>‰6¹¿C?á)(Ü~VÙ?Ê>‰6¹¿C?êÄ5ÛÈ×ä?©ýKË©ã?Äï(Ü n?©ýKË©ã?ç!:ÝîÖ?¨—Ÿts5?ѼåŠD"U?¨—Ÿts5?äO]¾Ö?º5'Uyü?ë:Vì(K?º5'Uyü?£Ë…ÓRȱ?°»lAæ?îÃG£Í5?°»lAæ?ЭÞ§ã?³Ü1pÉ?ç©z¬€?³Ü1pÉ?µÍ#_°³Ÿ?œToŕ?íF["%fl?œToŕMIXED4FGL J1217.2-2500¿àQÖs-ò@B›ÿñÀ;k$á`؈À<Ô¯«SÖA@¶E‰÷æ@>¢'vge?ØfÜ­ë`6?æ—r½·±@
›©ÄŠ,?üüøÔg Î¿èPä>X€J¿á Îï¼¼¿›à®^«9³¿ãêv–_Rv¿ïÿà•V"¿ïÁa)ÃÂUNASNone?îoý€Äx?­#‡ó{?©(Çmw?­#‡ó{?ëWn3PK?»peû~ÞO?¢GÏ2¾Õ?»peû~ÞO?íioÞgÝh?ž'ÛOí4>?´´
œûÃ?ž'ÛOí4>?êÀx~ýó?¢ÿ–³8,?Äþ3'?¢ÿ–³8,?ì]é<š5?ºó¿ˆt5å?½¶/†U?ºó¿ˆt5å?ÚC¾Uæ?ÐÝQº\ݧ?âÞ ÿÿÕ
?ÐÝQº\ݧ?çã.‡ªH?¶Mš·Ãu?Ð9£Ìð«q?¶Mš·Ãu?×!ª}J68?·a6K4""?äo*ÁZää?·a6K4""MIXED4FGL J1218.6-1049?á°òA.&7@Iœ,ÂãÀ:´'QžXÀ<L#{/KG@ؓ…ƒb @ßoijù—?Ӑ¡7óŒT?á6,­4¨@ó÷ ]m™@áÞõnW?ïÿ·hª¿Û'{°)©¿éhÚ´ìÜ7¿ð?ïú—á2µ_?ïÿ¢bôUNASNone?ïþ 6
O–?9<ÞÍ<?%üœCÁ†ó?9<ÞÍ<?ïݺm-Ð?‹="`p"Ø?q"Ék‰ßê?‹="`p"Ø?îWó')*?žÀ+9ª?ª€ÆðØ?žÀ+9ª?ïÿ&]%¹½?À'თ?4Z¹¶»?À'თ?ïû¯X5Ž?Uf1œ_
®?AB xìn›?Uf1œ_
®?î{…'"÷!?ºä?°8?¨G§Ô,Øõ?ºä?°8?îmRÄ??ž¢÷¤,hÀ?®ù*ãSX	?ž¢÷¤,hÀ?ïàSѧF?v¸&|µk?o¬.ÛÙYÌ?v¸&|µkAGN4FGL J1220.1-5558¿ïåFM8ºS@ŠŒ›"UeÀ9é'Dé>À;î(«ð´3@ßG`'»)@µ'-lJ?Ã+þ +ïr?ţܾ‡d¹@Á\ºT$@tÔHD:?調.%­¿äëEÉ7ìÖ¿àÒÿ¡‹U‰¿å(‹¤äPw¿ï±‡¿g¿ïýyb—yÚUNASNone?ïÞéGµSè?ky!Ç(‡®?p‹\x*?ky!Ç(‡®?ï¶úÑJ"€?ƒÏ)uӗp?'AK¾15ý?ƒÏ)uӗp?ï²ëòyQ?'õÎæý?œé¢ùß?'õÎæý?ïwFTfùM?sák¯nç?'5o±:`?sák¯nç?îäc½ùJ?ŸæÞ/›…?¡¹ÏCD"\?ŸæÞ/›…?îdbå…?³|ÿœê?®	¹Û6$³?³|ÿœê?íEhDëu?§hßyŽ˜?µÔ½ÚÊ?§hßyŽ˜?í\<ït—'?˜okËzô?µ"É7s?˜okËzôAGN4FGL J1220.1-2458?ÑdêüÉÐÕ@B­³Ð|"¶À:œ€šÅÀ<c«Ø`~Æ@ _ºª@TXÍ ¯£?ÀmÓÃ-¿‡<3•ŒL]?Ȭ| 9›Ø@Iۂr6?ë|¿€^	¿ä)ôÆ)¿â<½ ‰ø½¿ÜB_ !¿á¡–
W¿ÕM!ñÂO›UNASNone3FGL J1220.0-2502?ïûŽgr'(?4g/]É8:?AÆaüïH?4g/]É8:?ïó/аº¦?[—úiß]ñ?Y ^º"Á?[—úiß]ñ?ïøN3¿ ??]ç8Q¯?OúÆg˓ü??]ç8Q¯?ïõŠ‰côû?:DB´Wœ?Têí'—êß?:DB´Wœ?ïöVX{?JLD)'?SSé½òŠ?JLD)'?ïËùn§Ž¶?"AìñŠè?zH[í-?"AìñŠè?ïûô­Ð?Rikíь ?@-L•U?Rikíь ?ïÙ «~?`9·©Ù`?soñ½
¤¬?`9·©Ù`AGN4FGL J1220.5-2745?èûYuš¿g@AMçê_"ËÀ:zÉۀĶÀ<>ðd‰Ø@wQ-=¿@¨tBÇû­?ĕeTB¢?¶Ñb?ïf þ'@Iòµ>»¨¿é­ûPm׿Þ†nCªz¿ìbÁì!¿Û"fy±œÆ¿ìÿ»Ëǔ¿ïÿ\l¡UNASNone?ï¨O?‹ä®?²HˆcÃ?…ì0—8"?²HˆcÃ?ïêð7ØV?os?'?eb"íšd?os?'?ï'|=#ˆ,?‡^³B Ü¥?‹ ðº'?‡^³B Ü¥?ïè'
Ëz?P">K&?gâ}æ>@?P">K&?ï–ñ/qv?ŽïçR5â"?ŠC´*˜M?ŽïçR5â"?ï¥Ür÷?üÊ+Ã?†¸ N1?üÊ+Ã?ïE`úÁ§«?'¼ÎÌ+ç?—Sà¬òt¤?'¼ÎÌ+ç?ï*‰1}·¢?‰ö°ñe6?š®ÙDzÌ?‰ö°ñe6AGN4FGL J1224.6+7011?êõD'@GaFÜ]cˆÀ:\H»Z´À<PÑæAq@ ­'ÐÅ@7ºœH ƒ?¹Ð­'ÐÅ¿¡ÊžÕ˜£?ââuuÍâw@]/ÆO?ïÿ
¢q›¿æFIlÊ.¿ë ²Ý¸Wu¿å¸
ñâ¿ã8?!(οïÿøþÙå9UNASNone?ïÀÔìiÿ?±t¥E–¯|?•÷rm¨Ë?±t¥E–¯|?ïó¤IöÄ?W'|½•u;?X·l_o^?W'|½•u;?ï˜k&ºó?Š1uNþÄ*?‰å6t2S?Š1uNþÄ*?ïáeìÕ%?V›ÿþeº?nšs;?V›ÿþeº?ïÝ×.$«†?²¹ÅmæÃ?qi
†ôØ?²¹ÅmæÃ?ïÎnc§€?xJàMYv?xÈÎYœ?xJàMYv?ï‹ò¦ók¿?‹žâ¡¸=?V8Ö<6?‹žâ¡¸=?îôµg3—?,ú'‹f? ´©Ž…ô‰?,ú'‹fAGN4FGL J1225.9+2951¿ïê/Ÿ¼¸@Tñw[0À9'7 þ}IÀ<@̺XV@±È,)(Ã?üT¤MQÂ?·JRŸ	E#?Ú÷FóÚWÐ@"Ðàm"@±a5$$"?ï•¿,{3?ÌïÒ Ì=Ü¿ÑPLH­î»¿ÝΌ 6즿í]¨QÃA¿ïêo_‰RzUNASNone3FGL J1225.9+2953?y?ÂêÌK?¨—Û3¯êE?ï̀zJA?¨—Û3¯êE?Óm›ÓŸhª?ʩߕ"ê"?æI20K«?ʩߕ"ê"?·J\ȃ?¦bN.Û6|?í´fÆÕß?¦bN.Û6|?¤ÇuR›?'Ë,.â5?ˆªÖO?'Ë,.â5?r,kàý?šÙìÂvâ©?ïÛ§("ˆì?šÙìÂvâ©?¹§õÊ>t|?ÀA?VhR¶?ìËF¸1p?ÀA?VhR¶?§Çæ³þŸ®? 'íÝã?"À? 'íÝã?Wõ¥¯/í?PÓ;yoV÷?ïô-fj˜?PÓ;yoV÷PSR4FGL J1226.5+3023¿•ªÄuv‹@TéªÍžƒäÀ;A§
›duÀ<x
c0Q@S͍'ùg@ÁòÜ+¢?Ì¡›†-Öþ?™]g—Çe?È01¡Õ{@#r ÜY¿ë^¿¨÷Ûn¿ÙhòÝ­š­¿Ø@ãȑտëÞ
Â5o#? æPž`~¿ïÿ›¡[¯ÔUNASNone?ïüßës½"?6ábYô?9¢ñÀÏÏ?6ábYô?ï÷£¡ô÷?TBv|qJ?Qò¸Ù'Ý?TBv|qJ?ïΉËì¨?x¨´æcc2?x»} 8÷ó?x¨´æcc2?ïûô7þQ³?0Cq¶s3¿?@/ (B1ç?0Cq¶s3¿?ïö"cþæ?Sw<4á=?R÷9yʤ…?Sw<4á=?ïÚLð§%&?wnGnôs?rهšu?wnGnôs?ï‡4;¾>Œ?Ã—Ë·n¯?Ž2ñ
Á?Ã—Ë·n¯?ïß
¼"§í?j+^¡ú§Ù?py"
(éQ?j+^¡ú§ÙAGN4FGL J1226.8-4907¿î}+¾ŽŠ@+ÄÞÁÁ×À9}ÎéöÀ;PÜ¢b–@	ÛhQx@B Ž€a?¾ß¡:ͱ?Ç=ýçvò%@H™|=h@@
EBÉ(R…¿íóû¶Å?ÎâüúgØ¿êO"J'°¿î«ØáX&¿ïú	.Îõ?ïá c¸6=UNASNone?ïø£Nh¾?a"£¼ÚO»?MrÆpïãy?a"£¼ÚO»?ïÍyñf<Ó?ŠæPY8?yC5">d?ŠæPY8?îô—ClÖ?"ˆiGK«ë? ¿öˆY–¤?"ˆiGK«ë?ïîíöh?O¦m9¶":?a	ïÏO™?O¦m9¶":?ïÈ`ˋò?‡ëN©ÊJ?{Ϛ:àòæ?‡ëN©ÊJ?í©‹žHâ?»34=|ì?²³£u^p?»34=|ì?ëtD¿'i¹?¬Ö#ØÁ?Â.íºY?¬Ö#ØÁ?îøã·Ršµ?"LMzK‹? qĈBŸ±?"LMzK‹AGN4FGL J1228.0-6918?ç¢H(ÛÛÀ#âOëОÀ:ÇM~8DÀ<)©HcF @Ùe4%m@o«Ú
ýð?ËT3]û]Ú?»(‰Œ\`?ð•¢y<,?ý9+€À…?íKT'
`ç¿èÿ §?tŠ¿ä|<& ûù¿ã.÷ϯÖ¿ç…ý_çœ1¿ïŸ€-·É0UNASNone?ïõ};¶~?z<ËÒÏ?Uá›ÐÓZ?z<ËÒÏ?ïÁ܇¤B?Šþÿ¾&ž?¼›?Šþÿ¾&ž?ïã—.â?h'qéá?lhúê;M?h'qéá?ï¾yòךÓ?_n"´?€aƒQ¨o?_n"´?ïõ!F:¹?T³Çí8Ü?U½tό?T³Çí8Ü?îà`	ÍV?¯Ø…<ÀO¼?¡þÒÆ¡?¯Ø…<ÀO¼?ï£$ãöE?ˆÇŠ¿ÎM?‡>öÔÀޘ?ˆÇŠ¿ÎM?î«›Ø@Ò?•JïSô?¯¥FA ã?•JïSôAGN4FGL J1229.5-3048¿ßzÅ	A0@?Ó ù	kºÀ:óD{ZrÀ<e†Üþs@âƌì¸@»œ"á?ÖØ­Áä}?ÉäbÈ!?õH(¨•µß?ú`ŒzLL_¿Þ)Q¨,Y¿êR½<6¿Ûœ²þšz?¿çEa-¡¿î	‡"s\¿ïêvUNASNone?ïȎow·?v¹Ó'a?{¸È7) '?v¹Ó'a?ï§/aõñè?ÜðæšnÐ?†4'ê?ÜðæšnÐ?ﱁþ?³ú4p?ž‰×0ˆF?³ú4p?ï~Ô+Òv?r>R
¥mU?%zå±J?r>R
¥mU?ïˆØÊ9¨?ŒÉOî">?ýÉÔPÍî?ŒÉOî">?íÑW~'?¸€Û×èX?±uG^Ió?¸€Û×èX?í~ÏÍC{f?£…"èW«?´	•ä$Ð?£…"èW«?ì­Œ?¦Ž~ãQã?¿Š"›—m?¦Ž~ãQãAGN4FGL J1231.6-5116¿Ïe¼ðX:@&÷\òI^À9ZZ¦>ÊÀ<z>ŠJ@F:ωÀ‰@fû_‡O?¸4€·å#?æj'ào–ç@'•€^_0è@¾€JGÖ?ïÈÜ}Cø}¿½Þ½åÿ"à¿äw݇/3Ê¿ïi'2t¿ð?ðUNASNone3FGL J1231.6-5113?|€°BÁ.?¡zžøå@?ïÇÌþ~~>?¡zžøå@?²qz'	µÞ?°4Y'Â?í±Ð­µô?°4Y'Â?Ì7#øi?°
:~5x?èòÿ÷æ?°
:~5x?—U!àôxÃ?Ù­uë ?ïEVðÁbz?Ù­uë ?šËi®Ã?³.•rK)¨?ï)¤²¸Š²?³.•rK)¨?‡j}ʵ?Œ¼™ô"YA?ï¢V	T›?Œ¼™ô"YA?Á¸@ïø?±@áF>nI?ë'ïþDü?±@áF>nI?$(ãO›˜ø?$"Á/ÿs@?ïþ½rR?$"Á/ÿs@PSR4FGL J1231.6-6511?çÀ­Ù©TÀ6Ÿ~µè…À96‰@†
À;9åèý"û@ٝÃõ¸©@"dEú¶?Ân D2Ò?ÝÊBÄJÈ%@ɝ_÷·\?ÿ'—¿ïÿÿ)@k*?ïÿþˆ0»Š¿à¿"àT¾ô¿êŒ@À}¿ìý¢yM¿ïûîיåUNASNone3FGL J1231.7-6513?²Bî¸Á
b?½&pEüþ2?í·¢(çÞT?½&pEüþ2?Â$cl`üD?¹°ÓBÃÛ?ëvç$çÀï?¹°ÓBÃÛ?Ë®š@Í>{?°)_ß^€Ü?éYoÌ°a?°)_ß^€Ü?Ó±Wéÿk8?°ñHl«Nù?æ'TJd?°ñHl«Nù?´"ºÍ|è6?Ì __к?ímˆ¦yžI?Ì __к?Œ(c­k¶ò?à¥VB*=?ï^qWe?à¥VB*=?¢\V"Po?—ZÖŒv?îÚ:—'½¾?—ZÖŒv?‹ÿŽˆFõƒ?ytebôV«?ïŧêj?ytebôV«PSR4FGL J1231.7-6653?ꈛ¥7‡ÀcËďªÀ9ðh¬'ÃâÀ;G¸ü5p$@ÕúK`%°@¥EŸF'?Ô͍Ý"ÛL?ãÂÜSRl@	ôŽ:!d@!$‰w7š?ÚþcGοågÔôó¿ì®Êžc˜¿ëiäñÒÁ¿ð?ïþ× ¿UNASNone?î&	…ÿw´?²ösBe?­Ÿg¤T¿?²ösBe?ëáÑ°{!M?Á|fýR7?Àx¹>zË?Á|fýR7?ë~÷D«?©G¢ßKQ?Â#ÎïÅS?©G¢ßKQ?í½±ËXrL?›ÙýtÐÛ|?²q¦T¡?›ÙýtÐÛ|?ë6ÑaBKe?Æzïæ¾v¯?Ã$ºzöÒk?Æzïæ¾v¯?ËÑÑ엡?Ï1¹FÄF?é‹¿ÄÚ?Ï1¹FÄF?ãr¤.ÀT;?¸
ùÁî ?Ù·¢WŠ?¸
ùÁî ?϶¯áÑä?¾p~‡a<?èT‹†ÿ?¾p~‡a<MIXED4FGL J1232.1+5953¿ÄMÐ*ØÏB@L‰ÄڐïÀ;½—¥¤À<³Ùý7@õH&4r#@	=·ä{õ?ÊÈü]´¿®RºÀŽX¦?ÜüϞä1B@v=}dá¿ð?ð¿í9~¦Ï¿ïÄ_@¿ï0_y[X?ïGâ¢w
ÓUNASNone?ïúX·¸NÍ?tŒÚ߁$Ä?F ÷¼pÊ?tŒÚ߁$Ä?ïê	uÆ?x\H_¨!Á?eöôeÝri?x\H_¨!Á?îvÔ}ù³"?›4jZ£²?¨'¸õ*Ð?›4jZ£²?ïë0Ÿ§r?Vl<0‹LË?dÏ``Ìù4?Vl<0‹LË?ïþD:[_f?A‹2‡Œ«?+¼\¤'é+?A‹2‡Œ«?ï MavU?°ƒÃjò?›öSԟqM?°ƒÃjò?îˆÚÄ~—?-=1+‰?§rS¶^Áï?-=1+‰?îåEÈÞ? §f;íBÃ?§á«§ÊE? §f;íBÃAGN4FGL J1233.0+1333¿ÁVUÑ\˜K@RðÞÑ·À:ü˜lrðÀ<B½=ã^@&Ø,ý9&@§ …±…I?Ãd´ CŒ?Ìf7AŠ¹Ø@ä†&ö@Õîßq??ïóçÞ¡
§¿ÖŠîü!¤¿åß«Ì¢¢¿èH'_ì#տ뒥2.¿ïñ">¿UNASNone3FGL J1232.8+1332?ïèûÛ>eÒ?aP!)NÊ?g$Èyex?aP!)NÊ?ﺭ·?ŠÐÀµ,ì?T'7Rb0?ŠÐÀµ,ì?ï§þ<9ã?zÆ3NU?†pø—.?zÆ3NU?ïEPOE?{Éån[¶¶?—]ö-å\?{Éån[¶¶?ïpþÈÀ?…Óì˜ók?ˆ£Àvî—ú?…Óì˜ók?ï¾mÛÈ
?¥é*¾?ŸÈ2M½?¥é*¾?í"z2Ì'?£‰5š×âI?³Ü.gèÍ?£‰5š×âI?ëÒ\O¥ô`?¥QPInÏ?À¶ŽÁh.?¥QPInÏAGN4FGL J1239.7-3455?ȵìx04É@;âbS—À:ÐDñ¡˜lÀ<Bãü";@äÊ-
O9@%1"Éÿ?Àq2GOõ·¿³d$í ,?ñËý™ô2@Y±=¥'?Ò
»Då_¿æ¦F…öN¦¿ïÿô¬å¦¸?ïýŸêÁ¿Ñüê
î¿íIhÉíõ<UNASNone?ïüßÕú.@?L)ýa{ô?9QAn½Ö?L)ýa{ô?ïò½Ýñ?`FŽ|&Ž'?[âƒÀ+æ ?`FŽ|&Ž'?ïßȳɬÃ?wfT-¸Ð?p¦º†?wfT-¸Ð?ïÿ†…üÀ?VŸõ?o1'$n?VŸõ?ï÷dÈ×tÆ?L>BO©DÉ?Q6n_ƒx?L>BO©DÉ?ïƾ(Up?ˆ'XHF]?|ó úC£ÿ?ˆ'XHF]?ïË'¤Îp?€bðˆªÚ?zxìGãó?€bðˆªÚ?ïô4YÆ<\?[£@>º÷÷?W—Lìy†Æ?[£@>º÷÷AGN4FGL J1243.5+5311?ïûОœ}@Oñ\(öÀ;´vTðóÀ=C'üÇf@ cõpÚވ?þ*(,nô?ÔªL¤ô@¯?±Ž%È¥j?ÞzÊáæ'@x8֋<Š¿ë$ñ`®—¿ì.û€"dü¿µ™ÆÿÈ"¿Ô*¡OÆ¿ïx×ì;?ìÄs'-Â0UNASNone?ïþ.Au?'Ó\÷~Ìß?-å8±-±?'Ó\÷~Ìß?ï÷žvðnµ?RnºÁ\?PÃ¥ÓEƒ?RnºÁ\?ï©A,ùÙ?vh‰Ð§?…¯´¾,-Ø?vh‰Ð§?ïúIÁ®ÐQ?7Ї…bbM?FØúõæo?7Ї…bbM?ïÿ KúÕI?‡X0Ÿ(?ö‡öèCU?‡X0Ÿ(?ïÞÃË"?r} Õ-†?pž{{'t'?r} Õ-†?ïÄ­UÛv*?ƒñ˜ë2<?}©UF*ê?ƒñ˜ë2<?ïê´˜|Â?[Y&€@,?eKñƒ5?[Y&€@,AGN4FGL J1243.7+1727¿ïèjÃJö|@T
¯%;À;9@À<Ù$H¸@ ‡Z$ää@\ú&¢+9?Å´ØÏå[¿¶9÷GŸ¦Ï?壼gú»?ù"€€Ce¿çGìþ›{ò¿ìDåýö:"¿Þ5'm,S¿Ø쮿p˜Ä¿×`^l¢¿åIÛ¶t›³UNASNone?ïü3劳Î?4nè&œÀ?>`Ñ»™Õœ?4nè&œÀ?ïé.,c5Y?kæla¤I?fÑӔ‹–?kæla¤I?ïëÞ)/h?otBÓRb¤?d!ÖÀÎÇ?otBÓRb¤?ïð 
ˆ÷?KÀà#¤§?_¿åa"Üt?KÀà#¤§?ïú˜õ¯Äÿ?=ÞKm¬ßa?Eœ*	•2]?=ÞKm¬ßa?šQØî?™>6²ÉµN?Yuؘ_?™>6²ÉµN?ïðÕë"rì?pέ¤GÛ?^T)ؘ7?pέ¤GÛ?ïQ8í1q<?ŒðLý¶Y?•Øâ`±q?ŒðLý¶YAGN4FGL J1244.3-6233?ëÉó˜Wi?Ӝ?{Àë˜À8Y®4[Q_À:Žž @7Û@&ªfpwa?¶Ž±3>F?º×Eâz@ÉÉã
€ò?ø8DD}ˆl?ïÓ5!	†¿ÆgÆ£=q¿ãg]Ý*é¿æÞíášdE¿ë›@˜vƒë¿ï.
ß¼"šUNASNone3FGL J1244.2-6227?ìe:<ýS?Áã2ïÁn?¼Ö.xe?Áã2ïÁn?áÿ²œí-?ÌÛºàU¬?ÜšÆ%¤æ?ÌÛºàU¬?ã £‹•A?´î'ªø??ؾ¹ÚèÕ}?´î'ªø??àMݕ5˃?·4WR²?ßdDՔhû?·4WR²?ÜuÛB 'l?ÈC2£BÔ?áÅ^¯ìJ?ÈC2£BÔ?¶ÅÂiâëÊ?À9î‰òñ?í'G²úœF?À9î‰òñ?ãùydߗo?¸×2Åã?Ø

6@Ñ#?¸×2Åã?¯µLAeê¯?U›žô¥Ã?î«;é¡U?U›žô¥ÃMIXED4FGL J1250.8-5424?Ó«³fþ@ î)Ø@žVÀ:ƒø³o.À<Ï<é•Z@¶Nií"@qº?À~ÀzY
?"0'—|<?хX.•>Á@•x´Ðì?ïÿdd-§¿ÖЏ$Äì¿æ8õ³¿Ù¾@Bo	¿éŽÌܽ¿ØˆUg"UNASNone?ïìþH=?`ÆiÕµjb?cüÏ\ë²?`ÆiÕµjb?ïß8o]0?x£=QX.?pcÈ1˔¿?x£=QX.?ïÎjô7d?t-'F-õ?xʅØÆ"?t-'F-õ?ïí¹ìËDâ?Dà0öÈäû?bFøAý÷?Dà0öÈäû?(œ‰í?ƒÞ–ÃØ0?ˆ5Ύ°í?ƒÞ–ÃØ0?îòëzÀn"?¬*…¾,ì? ÑHU°ëÙ?¬*…¾,ì?ï5I=>
?"9e³UZå?™VÜ6 p»?"9e³UZå?ï¦0¶0í?põúºéý?†sÒUdðÌ?põúºéýAGN4FGL J1250.9-4943?Ô"Îíʄ"@*M~Ë·ù×À9ñ¿³ß•ýÀ<8#;nk@'.íÿ"@ÿCB?½jtËáY?¾ÖÜG©ã@Å$aß@iˆZ?ë†+'Ëöä?ÚAžlK¿äÏ?mÔñ¿Ñô" áw¿åˆë–¼o‡¿ë:ÿ[ë8UNASNone3FGL J1251.0-4943?ïý†/¦Ù?)Á5f97›?3΂Í;Ú?)Á5f97›?ï×ÿ#OB?|ÕëeL?tn=
ù?|ÕëeL?ïó"áÈÿ°?]¦t¼4?Xö;ìÏP}?]¦t¼4?ïÖÝ&-³?Xk¡H'I?t'lã¦Øš?Xk¡H'I?ïø["?K8æ…Ãip?OïÓ)rM¸?K8æ…Ãip?ï
Ës~'?¦å&)È@ð?žFœq;!?¦å&)È@ð?ïݐ*Q…?zi;aˆ?q·óM¢?zi;aˆ?ïpaÁ)ð-?}M?ÇíÊ0?'óÇÒ*ôd?}M?ÇíÊ0AGN4FGL J1252.7-2520¿À~%¬¯Bp@B»ýq°GÀ:£9Œé‡îÀ;ëô9rè@"<͐Â@RoFøÍ?á¥ô@")›?ÕBTcY–Ÿ?ðèçÖyõ@…ë´½·¿©uy~Çc?áOmŽo¿èM_.cÀš¿ïqKÞ'ñ?ßÎùã0fz¿ïÿüÉï£UNASNone?î~¬j?ƄOúª?§Î¥l?ƄOúª?ïð‡#ö?g›^¬døª?^ñû°½?g›^¬døª?î³Ð"Üg¹?™¸›â¥?¤ÂýÎÉèq?™¸›â¥?ïþOôŠ?#ˆêbõo?+³ª¶3?#ˆêbõo?ïÄøçv¶?• ›‹I:?}ƒŒ8öR@?• ›‹I:?ï´P³2B?u¡ VÖ?'ëÓ@åéu?u¡ VÖ?ì<> eêÚ?¬&;èü?¾üЩ.?¬&;èü?ïê±åí"?dÁþÑÐlg?eNªz6X?dÁþÑÐlgAGN4FGL J1254.7-4516¿×G2¢R¥@1—Ö[åÚÀ;…Y#‡Ä…À=gû'@ RTN‹Ô4?÷%
`¬B?Ö¶N›™y
?鎥.i@g›\è8c@ʈˆ¥*œ?ïÿá'¢±¿íä‡imP?܄",tþ¿¿)¤i+g¸¿èý0½b ±¿ïÿýawUNASNone?ï]"k ô?"RœEužö?"[²'çµ?"RœEužö?î¹µö>»?«ÌS%"?¤d ×²R?«ÌS%"?ïUÃHc?¨–ú'^»?œõG¤¶+–?¨–ú'^»?íé7w?•-š-mjt?°¶GOý?•-š-mjt?î¸F'¬—M?¥®Ô—±?¤{…6‹,?¥®Ô—±?êz7x´"?Ê
bAQ?Æ"-¯³?Ê
bAQ?ìòx5éæ?¨{Åz7?¸l>W–¤N?¨{Åz7?ê´hŽ£‹$?³Ó¹n'?Å.]ÅqÓq?³Ó¹n'AGN4FGL J1256.8+5329¿Æ©D÷Á@OÏÞ灃ùÀ:A'½µÕÀ<2ºOò†›@¸b4þdt@@'w?¿JriÿÎ?´Å–¶eW?ñ~@'7|n@Ï&ݺZÚ?î!၏·™¿åPʽþÓ°¿ép¿ñ7n¿ä–fr•I¿ïÿ+Žúg?ïæG\µã|UNASNone3FGL J1256.7+5328?ïӏڱšu?¡ž«EK`?v8¡³e"?¡ž«EK`?ïêc¶ˆ½©?h9gÒ7Ÿó?eœI=ˆç
?h9gÒ7Ÿó?ï¡bÛcàÇ?"'ƒçÈÕ?‡§IÙÂ:?"'ƒçÈÕ?ï˜u'ÉãÜ?u*!—Ïqò?‰â›|Xý-?u*!—Ïqò?ïSýO™?ž bڗp?þ{.¢ê?ž bڗp?ïR"Dps?¢Ð6ޕJu?•­wk9µ?¢Ð6ޕJu?ï\ýwö—Þ?tÉ#á6?"`PüšU?tÉ#á6?ìUvT4?«d°Wñå}?¿%TM_.d?«d°Wñå}AGN4FGL J1256.8-1333¿ï?A¹*P@H¥VHþÀ;-Þ5ªÜ¸À<ˆK¹ë@KsÙ@¤@}= t.?Çè£ØaÖ_¿¤—±U±?Üí7OË@ëFƏq¿Ø/›#1ˆ¿Ø‡Ø_ñ¿ëk!ÃI@¿ÄÔèå‡-Ü¿ál‹ä¥0§¿ïúlb~Ð@UNASNone?ïüö…OW#?/W¬.Iq?8KÖƒ?/W¬.Iq?ïòÏ=Èëõ?]–YNô?Za"R«5³?]–YNô?ïê÷§ŽFL?Yb´rmˆ?eXH~dƒ?Yb´rmˆ?ïü"³óÚO?#ûm‰êsû?;ba)IøW?#ûm‰êsû?ïóÔ:Õ>
?U¡ãóås?XW‰ïÏ{"?U¡ãóås?ïÄ´""ºž?‹9àG+w?}¥¶0•?‹9àG+w?ïÚv㮈?v¾ÚŸ2Á?rĎ)kæ°?v¾ÚŸ2Á?ïç‰mÙé?^)ÀL§?hv'®mç?^)ÀL§AGN4FGL J1256.9+2736¿ØÓcK¶@V+©¨–hÀ;äa1sÀ<£u»mÿ¸@á#õ[â@Š;WÄã?Ѭþüôã?Àå—IZè?èi®ðBô@ïƝޢ¸¿àf» Õx¿Õo"'`í׿ì•C~Yø¿Ô[€–é;¿ïýîþOü˜¿ïóöúUNASNone?ïîy%8|Q?pôçº?a†ÚøþÔ?pôçº?ïåDvì4`?{˜|ïWüÂ?j»‰
°?{˜|ïWüÂ?ïf'%ú?Šçlúîâæ?"-Û?P!?Šçlúîâæ?ïÊ^Ž^Z²?eÙü?zиè/þò?eÙü?ï§öHh›í?ËòImŽ!?†mۊ0Ä?ËòImŽ!?ï"?4H\?Ÿb–*×Î?Šþp/~M?Ÿb–*×Î?îÂêÙ°¾'?›?^I=^ü?£ÑRc<Iä?›?^I=^ü?îYÙÙ-`ê?›éRè¥Þ[?ªbbp™^?›éRè¥Þ[AGN4FGL J1257.0-6339¿ØTbtá ¼¿éO0«¼²À9=Åté¶èÀ;nããiÇ@8¯ÿ;_@˜«B8‰´?†'vçh?՘" ;^Ñ@
à×ò›?ï,é™BS¿ïýð@o[Ø?ïÁW]ßÚ?¨f]O³¿¿ä-Þ)ìb"¿ê.^¸; ¿îD$QîàUNASNone3FGL J1257.0-6338?êá	"q"?ÃÃ/Ÿrw?Ç´{Ûv;y?ÃÃ/Ÿrw?Õ¡UŽ˜Ÿ?Ê¢LƂ/ñ?å/U8ý³±?Ê¢LƂ/ñ?åõänK…?°ì¶3±œë?ÔÀ7#h÷?°ì¶3±œë?ÚvA•¡'a?²ç–Ò•?âÄß5/6Ï?²ç–Ò•?Í©'E,o?Ë¢3Ü{k†?蕶.¿tä?Ë¢3Ü{k†?¢èÎÓ:º?®»:'ìê?îßÁsIÆ?®»:'ìê?ÓY"…Ltg?¸©dø…Á?æS5½YÅÍ?¸©dø…Á?«ÙÉÙ?˜rØ*?îBcbƒ‹n?˜rØ*MIXED4FGL J1258.4+6554¿çÄÌQ
	@IšÏ¿ÆT
À;"åV0Ž=À=%|'K@\P¡X)ã@¾Àdß}©?ÌÍ¢à•+¡?'wÿ&L?Ò%œq».@Æ-Ní¤¿ê˜›î¿âQ–?òß0¿îÛK_ú¼t?çGÍ+¿ìÚǗæd¿ïÿå"m/®UNASNone?ïùAþä2U?hjiWðÚ?Jø¶!͙?hjiWðÚ?ï÷Uc"¨æ?R‡EAp=K?QU9Lº´@?R‡EAp=K?ï®çûb•?'zºÌf?æ?"F/ï ¦?'zºÌf?æ?ïü?1ªX??-þ*J\¸?>sÌá²?-þ*J\¸?ïõWëpÉ?V&5?Q?UûP4-€?V&5?Q?ïÞ­:òU"?rLOòÛ!?p©b"ãÂ?rLOòÛ!?ïµ9a~(?…/xéuÏæ?'¼1¡q*?…/xéuÏæ?ïìõY¼g'?`ÖÅwmì?c
¦ˆP­(?`ÖÅwmìAGN4FGL J1258.5-3406¿ïÅúÜ»¾n@<¾š,fXÀ:¥{ 1ίÀ<U /Äê@Æs—Qj×@@D
û?ÅÆ÷ܔ@?£uÌàÃÏ£?Ü0«½@>älP¶¿çž¬ÞšÕ"¿ã¯=šÀ5¿å>#¶e¿Ûa®[G¤Y¿ïúûHáb?ïNž=î"2UNASNone?ïúDpÈ??Bý"Ùz?G¾î]r?Bý"Ùz?ïòÄ¥ƒT*?]{«oùmÛ?ZvµT
Zö?]{«oùmÛ?ï×ÙÝÎÊ?s #'͘à?t"9Ø=?s #'͘à?ïù'9•í?9Ùê,%et?I÷tuÑ4?9Ùê,%et?ïñËlØùß?\)ÓßÍÇÕ?\i&:Îq`?\)ÓßÍÇÕ?ïÈ|AUF?~²GŸØ¡7?{Áßn%ú?~²GŸØ¡7?ïÑèG§‰q?€Ú‹®tÊ?wÜBè³4?€Ú‹®tÊ?ïÒÖ3uE?miø±H9?v÷"ùƒ-?miø±H9AGN4FGL J1259.0-8148¿«ò$üâßÌÀ2òã'÷ÓÀ:4·b|ØÀ;úÏ®ÿ\l@U-ß6[Ý@1Ze§#Æ?ÄETÈÚ#ø?Ö ÛâêE"@:¤vlmç?ù­q:)òm?ÌÆQ)³¿à*_"ÊÕ|¿ãnO3Cú+¿é°¥ŸaY·¿ïýá!˜¿ímî$nUNASNone3FGL J1259.3-8151?åº$ü¹¤|?ņ:柠‰?ԋ¶Œ·?ņ:柠‰?äš[ @¨?É–µÓOã?ÖËIÚ¿~±?É–µÓOã?èijê¸?°oîˆ/û?ςYÊTU?°oîˆ/û?è°Y'/ù?¦%I	æø?Ïñ>™÷@?¦%I	æø?ÇÖ{ø	U?À+WTiÓ?ê
aø}«?À+WTiÓ?Ä+k«A.@?ÆN•þô+$?êõ%/´p?ÆN•þô+$?ƃë9ˆ?±šÿßÊ?ê_8ùñž?±šÿßÊ?À¢I+/ò?¤—˜'G¥X?ë×mµ:4?¤—˜'G¥XMIXED4FGL J1303.1-4714¿îêaÑ3íK@/,e@ÌxêÀ;$zØä2DÀ<×ïÖ½—@?$š"v?ü)tˆhî?ÓÅá @è(?çruÓÁ³"@l¨ýº«b?ôÿVø4Y¤?î¬âžž?àdÀÿß¿ÜGüN¿Õ,HÓ
¿í߯Þ)–|¿ïü2JÕç(UNASNone?߯À}ð,	?Ê >¤UŠK?à(Áéü?Ê >¤UŠK?ÏVtÉßM?Ä㷆$Ù?è*b͈<-?Ä㷆$Ù?ä'œ_$[]?³~UÀWdz?×°ÇA·IG?³~UÀWdz?×_›À%i?°Ž"ÈÛmÓ?äP2ÀmL?°Ž"ÈÛmÓ?ÒlRà2ìM?ÌfXž™?æÉ֏æ‰Ú?ÌfXž™?¡Mµ=ڙ#?¥.¬•éš?îë$¬َ?¥.¬•éš?Õ<ËaV å?¸¤?/­Ò?åašOT¯?¸¤?/­Ò?­v	6S†â?˜)<G*¢E?î(Ÿl¨†?˜)<G*¢EMIXED4FGL J1304.6+0539¿åA—P$kÖ@QÂÀð À:çï¦ìhÀ<"®‹ÜB@£ÒW%V?þˆ×ªva?Շ-;!"$?àžÑç¾Á@}!"Î~@·ü—•³[¿ícƒ'ǁ¿¯^L€PJ¿Ûö î¿æ>$}㰔¿îxùæáK	¿ìšäó4?£UNASNone?ïîy;Äëò?cu—¡R?a†Ä0Nu?cu—¡R?ï£ÊhªŸ?ËÑKÍãí?‡
eߦðÏ?ËÑKÍãí?î¨ÅÓ©?'2ŠÑ0³?¥"¢Îem?'2ŠÑ0³?ï]J2u•{?wù›
R¬Z?"V¹³¥?wù›
R¬Z?ï½
Ý~ Å?ãx¡Û"1?€½H§7¿?ãx¡Û"1?îV{ēå?´Ï´]À$ž?ª˜C¶Á¦1?´Ï´]À$ž?êïÛohB?°Fd©§ø?Ä@'C†^÷?°Fd©§ø?ì»_f@?¢ò'V¤Þc?º'…ÄÎ?¢ò'V¤ÞcAGN4FGL J1306.3-6043¿ïþ6¿ã7ü@ÊصýÀ8kÚÜZ	À;"KâC@•û¯
t2?ü瀭9Š?±=z	3?ÝXʜpäo@)ð$p!Ñ@ú F˜7¿Á"Ê|æZ'¿¬\w`o聿Â1ÅIö™$¿ÝM1a!.¿êŸwßµ‡·¿î»úýŒ³,UNASNone3FGL J1306.4-6043?wÑ{¾€n??­hþ!&?ïÐä\ò…??­hþ!&?¬C–³¯F3?¦·ïêååÃ?î;Ɣ›ÐM?¦·ïêååÃ?É5ڏO‹%?­¯ÓH»%s?鲉\,7?­¯ÓH»%s?†]¢Ò»??{ÍÆl|I?ï¥Ê‰ðc?{ÍÆl|I?bÁ‰eÚ{g?YLRԏ??ïí>vª£¥?YLRԏ??ˆ^'˜?€å¬:Ý«Õ?ïÁöïØaù?€å¬:Ý«Õ?§ß|êƹ·?£šÈ[¸ˆS?î'18…?£šÈ[¸ˆS?—ñÅÿ­?ƒÊ7š'?ïÿˁPÖ?ƒÊ7š'PSR4FGL J1308.7+0347?ígŸSgC@P'˜ÜÛ7ÊÀ:¤''%ߎÀ<1ìVu@t1ñê"?üÞ£©½Ô?Ð*¤CkºŽ?×ØJ"]?@_"YÒÚ@k‡ÞY[?îT  ô×®¿·]
½ô¿Ê˜\©#O¿ããBZ£‹¿ì™ V¸¿¼¸ÈúÃUNASNone3FGL J1309.0+0347?ïåá†Ë¿9?h;ÂúÂ"­?jyCFÛ?h;ÂúÂ"­?ï'V@a	?–:²>½;F?‹jpõ™?–:²>½;F?î ñüuö–?"˯f@˜û?¥ðà<2š?"˯f@˜û?ï$©7¾«?~V«Ÿì/?›~
×P\¯?~V«Ÿì/?<Ù¥?˲V»	?Ÿ<t92³?˲V»	?îo³u@|?³ºü¯Ð?©4Ì"4?³ºü¯Ð?ë±&{óI?©H‡ëÌ?Á;f2Û¨?©H‡ëÌ?ìÚï—Œ? &<ÄpK±?¹/ "æ? &<ÄpK±AGN4FGL J1308.9-5730¿ë7`;K|ø@&ôàM/À:Ž 'F¿À<{æ*kä@—"§Šs?ÿü€ï~¨?Õ)ôzæ¦?Üxù!¶3@¨–2æ@¥¿p÷z? JAòh¾?ì¥~tz%`?Ö­Ò HÊÊ¿ãw?}ÄQ¿çæ!‡+¿ïÿž±0UNASNone3FGL J1308.7-5738?ïÈ·"Q?zÑþ¬²•?{¤7¾Ælf?zÑþ¬²•?ïD¦ÏÀ¦?@
íPY?—nKpåW?@
íPY?îdtSŽóM?™dÚHE?©¸ºÆ4ä+?™dÚHE?îÞUO+¦?ƒ¡I'óuÂ?¢«µ:ý?ƒ¡I'óuÂ?ï	wV"Ì?›i¼ãôÒ=?žÝ'ƒØw?›i¼ãôÒ=?ì#î$hô?ÁÕC±äÑ?¿.àŽÜ¸c?ÁÕC±äÑ?ë;‰¤À$"?¯Ô"§õ?ÃÙlÿmð?¯Ô"§õ?ì<ž€M2?¥¶mj¹?¾ý—Îq?¥¶mj¹AGN4FGL J1309.1-6223¿ïÈAo.?Ùõ7d›5%À8âŽÕñÀ:é@oUxW€@ÃWEa3!?Àø:8àò?ÚzÁÈó@ÔÌ?ß ?öˆÇͱտïô;pïVe?ïì´É Èb¿âÀrM'À¿êÍ»à~í¿ë'jxÅ¿ïÿ÷Ò4ÛUNASNone2FGL J1309.6-6230c?ÄëÂßä?˶¥÷~…?êÅ:H?˶¥÷~…?¶»¶d?@?±]Á˜!…?í(É\³h?±]Á˜!…?ÇÑP™dY`?±òŒ×—À¡?ê«Ù¦é¨?±òŒ×—À¡?¢ØŠ)Àìå?Û gbc?îÒw]HtR?Û gbc?¹–èììf–?ÐÕpEã?ìÍ"âFöM?ÐÕpEã?'ÔHó3ä?…"0KŠ3?ï´®Ü)"¬?…"0KŠ3?›sãèÍRf?š'YÔõŸ±?ï$`àž?š'YÔõŸ±?2cþ}"Q?*;¨¡dVs?ïý½3bê?*;¨¡dVsPSR4FGL J1309.3+8035¿ì÷Ø#à@BALD|0ÓÀ;*qgKiÀ<xÓâjÃÃ@y7OË@ÖÕ"õÎ?À°àÝûÉ:¿º÷Tføˆ?ú.Æݟƒ?÷Od¤šS©¿ËÊõQÓ²¿â¥ôñ¯e¿ì˜¦ŠB䁿ćœDCÒ¿ë†lËÛ5E¿ïÿ••_xUNASNone?ïñ¬͒?dphé˜?]Ĩ2ÝüŒ?dphé˜?îÙÆÞ~ق?¨½%ú`e?¢c'¦Õ?¨½%ú`e?ï{…FPq?‰Ž	=ww?Xí¿Ò?‰Ž	=ww?ïd›»²É?€aj^.½º?"¬‹ùBÙ?€aj^.½º?ï·ám:7?'°.ªç
˜?'¤¹Y9Ä?'°.ªç
˜?æd÷Ó?Ìçå'È­?ÓîÅ6ÄZ?Ìçå'È­?ï+tÜå}?"ãzôµA?š'd_Þ´l?"ãzôµA?æ‡~	Må?¾qˆÝ£x"?Òñíd5Î?¾qˆÝ£x"AGN4FGL J1312.3-6257¿êÚ²@âüÿÇÍùóv"ÂÀ8š"O…yQÀ:YÔQüL@ (~oÈ@¡Tÿ5Õ¥?Á÷ZjÔÌ?Šƒç€­:@I=Ùb·@C›`C¿ícþ¬Bê?ï(SÜ '¿á"æ".¿æS®h]·k¿çqß
¼òd¿ïü"à՘MUNASNone?ë
˔µÑ€?ÇxâæzÙ÷?ÃÈÑ­(º?ÇxâæzÙ÷?ï"öŽ+?¥‰±"¯ÿÎ?Ÿoa.:W?¥‰±"¯ÿÎ?âèVO0ـ?»âڀ>©´?Ú/SažLÿ?»âڀ>©´?î¡Òx2k¸?'l*íá¼À?¥âØ{ý]?'l*íá¼À?âùjnL¨"?υY®û‰+?Ú
+#f®Ø?υY®û‰+?ꎃæKpc?ʦ½õՕÚ?ÅÅðfÒ>s?ʦ½õՕÚ?ã⇺ý?¾DîS|¡3?Ùò;àðŠ?¾DîS|¡3?äü×ÛZë?Á1‹¾9·?ÖQÜIJ)?Á1‹¾9·AGN4FGL J1312.6-6231c¿é´÷UXïR?Ï!ٙŽÜÒÀ9QTsõ›"À:\Ä"Úœ@±öÃkO.@üØ:¿¯?Ґ`
à?Ü;\L‡@±žs.?üYçՑÂ`?åk¢E9Åô¿âŸ=ÙFX¿â1e"n"Þ¿âÓiÔ¯ð¿ë‰â!GÎK¿ì5?|í'UNASNone3FGL J1311.8-6230?Æ;1e :?Çæœæ™ì??êq3»æ—ñ?Çæœæ™ì??Úà14¹ó?ÊFрeÀú?âçe÷£?ÊFрeÀú?àŒ™bUúL?¶"èDw~<?ÞæÍ;Tg?¶"èDw~<?åŽà DK½?³k6­+ÀÐ?Ôâ?¿wh†?³k6­+ÀÐ?Ä}•Í1K§?ÂäêõE« ?êàšŒ³­?ÂäêõE« ?¡¡KôÝþ?¬…3Ñc–?îïÅë\/?¬…3Ñc–?Â}Mç6ö?®éñ¯\ó?ë`¬†8òC?®éñ¯\ó?³îö´¦%?¢+‹t?í'!)4Eœ?¢+‹t MIXED4FGL J1315.9-6243¿á'g^D??Œ¥šŒf]áÀ8rãËìÒýÀ9ãûó+g@Øçk´"@jZíŽ?ÃÌMß?;I§hå@ýœ¨?ãG_ºü?ämªþE띿§Ãހm<ˆ¿åwu³
"¿èœX@2õ÷¿ìPޓɡ¿æR£`—ÅYUNASNone1FGL J1315.0-6235c?Ù'~u¯b?ÕpìLš?ãq7@Å(O?ÕpìLš?Â)ByLG+?¿v´&㙘?ëu¯a¬î5?¿v´&㙘?ÖCÕ"ÂÞÉ?¶åQßòD?äÞnžœ?¶åQßòD?¦uå
Ð?'ÞzZuR¤?¯g·?'ÞzZuR¤?͘Dô•'x?ÖQ¨ÔŸÿå?è™îÂڟb?ÖQ¨ÔŸÿå?‰øöï<?'±Ü:?ï˜ëûÀ?'±Ü:?º¦‰—

?ªR¥`ĈR?ì«.Íþ¾?ªR¥`ĈR?<µšX¦Yâ?3 >i3vÐ?ïüiLõ§?3 >i3vÐPSR4FGL J1317.5-0153¿Û to²_@N&ìAÝ"À;DDfa]éÀ<ø0À'+ç@"¶'MÊä@Ôxã@¬˜?ÑùcCFPÇ?éizi~@}¯li¶?óQ½ØP:¿ïÿûÞ]Bü?ïÿØBKÔë¿ÐgbdÏ
¿é[O6Ÿ¿í"}¶98¿ïö¼?5õÛUNASNone?ɒM	žs?ɦ(8i?é›l½˜|c?ɦ(8i?Ðü"å#þ?ÄnóÚ›?灸=n?ÄnóÚ›?á@t-݉?´&±•C1?ݤDî?´&±•C1?¹Àßr…R?­$@/(?ìÇä¯LV?­$@/(?´–îŒ?ćŸÚY?ím<]B?/?ćŸÚY?®I'ížk ?¬˜°—`O?îfá
œf?¬˜°—`O?ă}ÿÆZ~?³QnŸª[²?êß €i`?³QnŸª[²?l½Œ<Èï?ZQ¨°)?ïãBsܵg?ZQ¨°)MIXED4FGL J1317.5-6316¿Û<Jwâ)¿áÄ* vmÀ8àÛÿo·HÀ;Ài;'@ÄØâ"Å@Ac?ÁÌm‰gÈ?â›êÂ+35@XÞô½²@Ì$'óÕ¿Ò¾0×@¿Ð¯ª}¬¿ËÈ©¼ýKñ¿æӉX=¿î<ƒß1i¿èPž¨øUNASNone3FGL J1317.6-6315?u[oÍ—?ƒ™ûÊ'_L?ïÕIý
hu?ƒ™ûÊ'_L?¹ïša}?±`Q	Ä
B?ìßBêÊ?±`Q	Ä
B?°‡?`'Zô?Ÿ™ã-›Ëv?íïû"?Ÿ™ã-›Ëv?ÀãhÝ0"•?¢=¾hP?ëÇ%ȳÚÛ?¢=¾hP?c–ëA"ŽZ? +7҄e¹?ïìi–ú? +7҄e¹?ƒa¿VÝx?…·‰™œI?ï²y§'ª?…·‰™œI?\öZw¶?|š" Ò7?ŒA?|š" Ò7?nÇPʒr?Z-»=šø?ïáo8Çò?Z-»=šøPSR4FGL J1318.1-3937?éÕw÷f"@6óNÒöÀ:O!Kª"~À;ø>ü•u@¹:"úžA@¡{j×?ÀR‹vÁ¿ºº¢Óª?ô&Ã$º@ϊxis6¿è€zC'üÇ¿çC{[¿å­Á±ç¿éEP6y8Ñ¿ïþ3ý]ŽQ?ïöW_¸LbUNASNone?ïá¢ÛÜ0? Èv;p™p?n]$‡?˜%? Èv;p™p?ïì/ÁÂ?mÇdÏS·ý?coóŽE¾&?mÇdÏS·ý?ï½óŠ?£H?'Íïfq¥g?€ƒr&ò?'Íïfq¥g?ïúJtÿl˜?7Ù)"—}?FÖ+á‹x?7Ù)"—}?ïï²Û2?k¯µ¶ïä?`MçVH[˜?k¯µ¶ïä?ï…¬+äØ?™²`;´I?ŽºÔî'' ?™²`;´I?ï: jâ*?Š]9Y!‹>?ˆ±wì&­‰?Š]9Y!‹>?ï˜nŸ¬€?'{j©GÆ?‰äXÚWù?'{j©GÆAGN4FGL J1318.3-1148?åÐ+›±™7@IBA¢a¿8À;8P©fÀ<þº…¢l@ °u±²ë?üÊØÞ¨—?ÌjØó!?¾úš ¹D@?õyç='@QŒõœNÖ?îåÑ0é­?ëEÅ.î*?´OÝà6r¿ç˜S~,Uɿ̙%•æ±¥¿Î•#éTqUNASNone?ïþòL@Óã?L/Œïùr? Û8ªºé†?L/Œïùr?ïîù:œ'¤?döƬˆoâ?aÅ%•d ?döƬˆoâ?ïìV YM
?e¾='QÍX?c©ß­'.r?e¾='QÍX?ïòÝ«t?E™JŠ?ZEÕƒì?E™JŠ?ïýÑó¹[è?0Òª0Î
=?1pb륙)?0Òª0Î
=?ï½Zãj6ï?]‡á¥I?€©Gô$F?]‡á¥I?ïã¸ýôZ?t,O–¤]?lGÔèæc?t,O–¤]?ï×ßÓ17?i·KºÍH®?tv&5˜A?i·KºÍH®AGN4FGL J1318.5-6352¿Ø®J«¿ò¸LH
À9ÿxǑúiÀ;
–}…fÝ@!1{{vn?ÿ܆铬ñ?Ò‡B)V?È'SV\ÿ?ñõ¿Ÿ½ 	?øVª0À'¿ês.0D?èRÔ¨ù¿êę!¥¿âŒ aßÄ¿à¢*aÓY¯¿ä²@¯rŸUNASNone?ïř§±_^?"ßqŽ9s|?}3,*¿ì÷?"ßqŽ9s|?ïB»ÉÅ0v?¡
Ô)ÄfÐ?—¨†É¿6?¡
Ô)ÄfÐ?îE‰Ñ¸´?Ÿèt¶ß?«§fóÀ[Ä?Ÿèt¶ß?ïdj!Ô2"?¿øŸTÁ¾?"r»Â
?¿øŸTÁ¾?îXî
Ä]?°³»°?ªq-ëì:?°³»°?ëĜQ¯Ë?É6Ë\ùïß?ÃÌ펹@Ô?É6Ë\ùïß?êÉ¢O9'ã?¯*¡Ë3ü?ÄÙvôv?¯*¡Ë3ü?éÞpœ'ñê?·ß¦è¦`ì?Ȇ=`8X?·ß¦è¦`ìAGN4FGL J1318.9-4556?ïö*qe@0¨àP7PÀ:kÒPšLGÀ;ɯe³¹@ëÙá³8Ò@
•Ât"6?×n†›e!¿ æÏ#á~?×ÝلÁg@Õ(eú±?ï==B€®¿è;/`Àµ¿êD~d^¿âÔãâh'¿á,Ãã?l¿ïÿùµc#¼UNASNone?ïó%úÄ	?Wà&(¶?Y´
¡(5'?Wà&(¶?ïҁ»	3Ž?³"²šÝ?v¿"uæÙ?³"²šÝ?懶7­ã ?'ïĽl"#?†Ü²Ȩ?'ïĽl"#?ïíAç«ö>?HŽa­¬?b¾0MÒ¨?HŽa­¬?ïÀã«?BQCä?òvm°2¾?BQCä?ïZQìB?¦¶]ØIï?œTµÄ/ŠÖ?¦¶]ØIï?î–<¹³"@?›lŒ[©?¦œ4g[pù?›lŒ[©?ï<ÔZ?ˆé(B×O?˜nt¼ž	?ˆé(B×OAGN4FGL J1320.3-6410c¿Í'w'¹4¿÷£ÄzÀ:ћh¦³À;cp£×
=@V%üi@·—Ù¥ù#?ÒO/¾¹¸?ãšb‹»`@ãI{t¥@žtGP?¼¤Eoóe¿Ø®ÿÿdû¿ÝSV>PοèöуòÖ¿ïÿý¡UûŠ?ïçÚÄç%UNASNone?ìZ'ˆÿ?¼þ"CµÑ"?½+s¿H‰?¼þ"CµÑ"?î\kP[@?¬j"|RÁ?ª9Jüâðú?¬j"|RÁ?êï`J˜€?«!Øo|Áp?ÇèB~՞?«!Øo|Áp?îÐtçU¸?‹ïߣŽÍ?¢ø±Š¯¤{?‹ïߣŽÍ?ەïô?Ώb$§Â?â5zzs†?Ώb$§Â?ÜА%Òw‡?ÑSCj?ᗷíÄ=?ÑSCj?ÛÚ\FQô?¼´é¹ w?âÿÑÜ×?¼´é¹ w?ã7ÊOL¡ø?½EuÉ
ƒ)?ِkaf¼?½EuÉ
ƒ),MIXED4FGL J1321.1-6239?Ÿ&Ï6Yd?oÒÃ(U¬À9F&yçL«À:=­P/Ã<@Cïò@Ï©@›çl‹C–?ÇmÍbôÁÞ?Ò7Ý ×ç@¼4 ˜ü¼?ÿ|ºñXw¿êö$Û?ﳨ~cÞ!¿äOÒ`_'5¿æ?_´Æq¿ì†väÝ¿ïÙ2ÁsR]UNASNone?Ù'm!ãÍ?Ñé›àÝQ?ã{¶Éo?Ñé›àÝQ?߬)›§2V?Ìï_Wîd?à)ë2,fÕ?Ìï_Wîd?ߧ*î¸|U?¶jü}]†•?à,jˆ£ÁÕ?¶jü}]†•?é,LXëuý?±WŽ @?ËNΜR(
?±WŽ @?»•Aº‰÷?À7ø̧Zo?ìWÝÈ®Á?À7ø̧Zo?­0qaý?µë¡bႯ?î,øéá/°?µë¡bႯ?Äá#$-˜?±û1Y×FT?êÇ»·6ôš?±û1Y×FT?À2((4žæ?±÷äuot«?ëóuõòØG?±÷äuot«MIXED4FGL J1322.0-4624?ëoP¿Nù§@0!y[5°¼À;¦v îÀ<ah#ÕÈ@õÃêûáã@ÿ$7í­?×Äzb?áƁŠY5@ÒõU'"@†Ùû3'¿ïö!Ÿ·ë¿¿èJ ˆK>?ïúÕÔ&]¿àwÍaGBµ¿èÝêa2Iÿ¿âG롤*UNASNone?ïð" â+?]®éyWç?_ÀÙê6©?]®éyWç?ïÊ'ÿ¡‹?'qçBZÍ?zö¶o±l?'qçBZÍ?ïj*À'ß?ˆÞ*<?'º¿BÆZ4?ˆÞ*<?ï…Q›å?zÚAß±Fƒ?Ž¸¹¡J2Á?zÚAß±Fƒ?ïʂNñ¢?}àph&ë¶?z¾Øz s»?}àph&ë¶?îíšéŒo?©&gºý¬?¡&Qfc²
?©&gºý¬?îO §Èäé?žŠ×)µ¦?«
õ†fg?žŠ×)µ¦?î_vÌÔÉ?£/`g_9ë?®Š"2³m?£/`g_9ëAGN4FGL J1325.3-5413?ïò³L"N?@ ž2~ØM4À9Д®xMïÀ;nS™Û@ŸOúi=0@¨˒:*?ÀQii¦î?Ð!û'©@ëÇ~¯2ˆ@1õ桊)?âìv Æ3«¿ÍMõVXÒ)¿ä=1NV¥(¿æ´äv]¿î^? ÿ¿h¿ïùÁ­UNASNone3FGL J1325.2-5411?ëZ'8.ù?ÄX»û:Á?•·D–?ÄX»û:Á?í—DHjŽ%?®3%Ý
¿?³EݾÑPY?®3%Ý
¿?큺Uο?¡&¾.0?³ò/Ÿ	X	?¡&¾.0?îw­½Å?'t~ë59?¨…$'Èû?'t~ë59?Õx°C1á'?ȔHè¸Kó?åC§Þg??ȔHè¸Kó?ßLŽìõê±?Î4çªëóÑ?àY¸‰…
¨?Î4çªëóÑ?ÚŸ7,*ð?¼å~rø?âò°diêˆ?¼å~rø?äy
ð%
ù?­bbèÛá?×
äµä?­bbèÛáMIXED4FGL J1326.0+3507?éÊ`!'Ã@SǘJAÀ:à=ûäÀ<Ð;êŠM@BúÑlð@¯_ü¿ÙŸ?ÄR†J1|z?À
W¬dM?ûL'"Ғß@!ü@­Å?ï4ãlK'µ?«5〇=»¿áËË]k¿á×>–¾ž¿ãúQjUß0¿ïýí5øàQUNASNone?ïþWë	´ñ?"_œBÏ?*QƒÙ–á?"_œBÏ?ïö\ÏJÖ?`Ñ«­e!ò?SF`õ«Ã´?`Ñ«­e!ò?ïñ<éÈä"?X U˜mo?]†,Ü*X†?X U˜mo?ï÷FëÌÂ;?6ö`g¦6¦?Qr(äí)`?6ö`g¦6¦?ïûÙ
çŽ??^|~{±?@›Èꫂb??^|~{±?ïܑ·‰)ñ?yž\>GÎ?q·$&s ?yž\>GÎ?ïåàqÅ?:?s±JKŽÛ?jŽXýV?s±JKŽÛ?ïë"æâ«9?SFˆ¯)?d{0'–Þ?SFˆ¯)AGN4FGL J1328.4-6231?辝 [Í?§Ë@ےbÀ8ÎÍÐØËÀ:d3çüÔ@9´ú,V@ü``'çÏ?ÌŞÛô2?߃>ÄE@|h½X»ƒ?ô#Ãy<
?ï°iS?Ã~.Ú²¿ì!-Aª¿ëÕÕßðëæ¿ïu'Þ—$Ÿ¿ïÈzη3UNASNone?ٞ	 Ì9?ÕK›ÃÚ#¼?ã0ûo™ã8?ÕK›ÃÚ#¼?ÆH‰&õ®?Ÿ›úz˜?êmݶ•?Ÿ›úz˜?á¯,NGÝ?´|¶ÉËÔ?Ü¡§cËpE?´|¶ÉËÔ?¼»ëº4?ž\ì8N°O?ì}~('ˆº?ž\ì8N°O?ПùmrQà?Ð}æ¡Ep´?ç°IF×?Ð}æ¡Ep´?ŒæQºÐ?"	¹«÷ƒô?ïìfðúÔ?"	¹«÷ƒô?Ò¾©7‹ ?·ª8ÐM'6?æ ±+d:p?·ª8ÐM'6?a‰ÒŒ·V?Png¢2½À?ïîëv
Öá?Png¢2½ÀMIXED4FGL J1329.9-6108?îsˆ7¿?ö&Ks›ÙÀ9œ§ktÀ;^iŸÖÊ}@Ù؅½™©?ÿà,%!øx?½ø+஁?ÙÒüÇf[@710ýÏ@®€™B†¸?í½ÚÁ'ï¿Õ™0þz™Ï¿Ó¥!ÂÈg¿ã¿YG¿í-¢Ðzw¿è@<›'Á^UNASNone3FGL J1329.8-6109?œÜšCdc?©£$:z'Ü?ï-ò›W?©£$:z'Ü?ÀëU³Þ?µl~+ëE?ëÅ9ª"}?µl~+ëE?Äd^º)?­`K…"ž?êæèyÑ}6?­`K…"ž?ÖÿÕsöƒ?²-0'ÝH#?ä€F¾x?²-0'ÝH#?xtØK[u(?›ŽÂé?ïÏOf‰f?›ŽÂé?… úVµÓ¾?ˆ#åÍ?ï©|À¥'?ˆ#åÍ?š])j¡M\?'çÝIq¹?ï-´ªõ•?'çÝIq¹?™Å
ږáo?ƒÄEÃo]?ï1בT"D?ƒÄEÃo]PSR4FGL J1331.3-3818¿ì˜ŠÛD@7ç†
¢À;›í0ðcÀ<zÝ¢w@€?ÐOŽ3?ýç½f?àEw¾}~±?Ò€U$õƒ?õYžfý@µ/â›Á?ïœÒhî#¿é­è j¿â–-žž¼¿Î±£Ñ€ç¿ïhey×\s¿ë_oÒ UNASNone3FGL J1330.0-3818?ïí"VX?s—;Òó£?bðݚDÐB?s—;Òó£?ïê¸Ä1?hcɹ
 ?eGîÀ`W'?hcɹ
 ?ï{óú@Öè?…'®W²<ª?€±êý?…'®W²<ª?ïàœ:2ÖÂ?R'%ÕOCß?ocÆb
º?R'%ÕOCß?ïï]—®w?^h"ö$À?`¢=p™:?^h"ö$À?ﺆ«7£?…ÑúF>×?^UF¯?…ÑúF>×?ïIð>kös?'ŸŸY_¿?–Áø7¨›'?'ŸŸY_¿?î*¯E?u?îŒuþº?Š^ÄkZÓ?u?îŒuþºAGN4FGL J1334.1-4154¿íÊëu¦Â™@4@Ùè>B[À:`˜I7wÀ;ýːŒªž@¸0d÷¦j@é̂$2?À˜PƒÑl¿¬6ð/U?ç¡»Áâÿ@ɘ
²¿ïðG€^?îqu‹u•¿ë\dŸ¼ÉJ¿âj´>`ß¿ÙyÂ,_Ú¿æÒŸ½J#UNASNone3FGL J1334.3-4152?ïö>»bÓ?l¦!^âº?SłÂóÉ&?l¦!^âº?ïߝ•/Z>?{…1À‡é?p15ˆŸ4²?{…1À‡é?ï¬Å±z6?*æ7ë?"ξsf™?*æ7ë?ïöAؽpä?>Ý8L'«?S|N^¢—®?>Ý8L'«?ïÌ2•uë?Œó3½†?‹ÌóSÃMQ?Œó3½†?ï0žsH!,?ª
Ø4Ú´?™ì1škv}?ª
Ø4Ú´?îê•ET¦~?˜8•8ZL?¡V«¨!ã#?˜8•8ZL?ï™u—†ÄÖ?€½Zy(L?‰¢š,
:€?€½Zy(LAGN4FGL J1334.6-4435¿ï÷ê,"|@1šP?³t6À:OÜ»WZÀ;þ†
˚ž@HÂÁ@lÇß'Bd?ÊWvßZn?ѤÃ,ºô?úßú Âî'?ùJ¡¶×¿á§úð̆V¿ç­czù›b¿ßí´ctn'¿ípÜá¿ÝwGʙ즿Ð}U–4ŠKUNASNone?ïé+LVg7?gó%AO ?fÔ³Ëôà'?gó%AO ?ï;ÿX÷¡?¢$ð«?˜€ýÝ?¢$ð«?ï&§6î²-?'÷ÎSÄ?›+'´^?'÷ÎSÄ?°Ð~?rËüûŽ5H?ŠW"ÈpÝé?rËüûŽ5H?ït'&?"NþüÛï?'|ü?"NþüÛï?ç«ÊÌAŒ'?Ï/šç^·?Шjg|æÛ?Ï/šç^·?ë	"\»¿?°ž6Ý?ÃÛvé?°ž6Ý?êeBûø?¶3ôëæÉ?Æj÷Ì™?¶3ôëæÉAGN4FGL J1334.8-3856¿Þ«ßÞ2¶ó@7("Æ£½àÀ:TqËõ6xÀ;í½îãx
@^¬ÛA@0!ùO×?ÁÀâ]Ø£¿¼jØE²?û­N'D?ú/}F'?ïôòñ#Ä*¿é-€¡{k¿äºïÀÛå¿æRuþ´ÑX¿ïöö¡²lÏ?î3Œ>½*UNASNone?ïÆ/¥Æ3è?Ÿ»[të›a?|è-8 P?Ÿ»[të›a?îL‰–ŸÇº?´Œða#é?«7fšO`?´Œða#é?ï&ˆÛ¹Ø1?'ÕØFúü?›.ä…U]ã?'ÕØFúü?ï"x1ñ?y'zCÆ/?Šáó±…L?y'zCÆ/?ï®VVÆ,Â?Žö(S?a?"jj=ö¯™?Žö(S?a?áèݧÄ_?Ò§iÏ/0M?Ü.D°wñB?Ò§iÏ/0M?î&ÛÙ?¡e°Á¥è?¯~/
þn?¡e°Á¥è?çø	8Z[ã?½Ç"Ž"ÿ?ÐíKH9?½Ç"Ž"ÿAGN4FGL J1335.5-4546¿ïÛ·"Í?õ@0ií9SÞ¤À:Ao.ŒÀ;û~ÿº_ã@÷ `ȗ´@ßݵR?ÈEF³î…?ч¾û¨ØQ@5]¢r†/@ÔPXÝè?äčc*qÄ¿ÖÛh›õ¿_¿å"øD÷¿æ"6 M}a¿ë½ËrY¹°¿ðUNASNone?ïTÅGÙn­?•ÜX'Žj?•gW\e?•ÜX'Žj?í›A9†3‹?­ÜªDÊzÜ?³%ö5ô%#?­ÜªDÊzÜ?îkÊÎð¾o?—1ˆÛ?©CS«ç?—1ˆÛ?íùí?ˆZ³$²?°7Žþß9N?ˆZ³$²?겧('49?¶¬0Õ3C?Å5c]·/?¶¬0Õ3C?àïÈT9Šˆ?πˆ6Öçê?Þ oWŒêñ?πˆ6Öçê?æ}áú}×?µi²#½Å)?ÓÉ<Q?µi²#½Å)?á­]Òw?°ŽÌÎ.´?Ü¥EÃÈ[?°ŽÌÎ.´AGN4FGL J1335.6-4052¿ä¡Ÿ:Ôxy@5;n.±Ä3À;^bMÒòÀ<…ú¯^&ý@!ì¿	ª@Óª6ŸÏ?Æz}ʆ –¿ÁÚèÄO%?õ-§¾Šà@ƒçÚ«?ïø˜,²²¿ìCË0ëZ¿ÚÌù"@F¿ï/<=Èã^?æÐ;·f3;¿¡Aµ)ßUNASNone3FGL J1335.2-4056?ïþi•ÝÖ?JS™n?Š½?)g#e¥?JS™n?Š½?ïìΖÀ:1?lñ~¢½?c1i)?lñ~¢½?ïÄa¾áҘ?ƒì@¿'™w?}Ï ozKø?ƒì@¿'™w?ïÿy¹:¯å?a¼)%c?ÈÚ°û'/?a¼)%c?ïý¬š—	`?9Òbêãòa?2›+TÞ?9Òbêãòa?ïŸ(ŠôÌV?'+²Ø§Bò?ˆ5Ý?]Nj?'+²Ø§Bò?ïÀôü/ª¬?‡_öÆ×{Ž?…ÇÞV?‡_öÆ×{Ž?ïöºA.ô_?Xëk˜Sf?R‹}™Ø1œ?Xëk˜SfAGN4FGL J1336.5-4655¿ï¼iûúÀY@.}â:óÀ:Akn
#ÕÀ;úž#lÓ@?£v'-•@éZD4"?ËZX¦ŠBå?Î[Ähû?ÿÓ8§z¢@ú…"áQ?Í&ý…Qc¿ä,È`›±¿éšãEµ¿äAÃ^¹ô®¿îq‹'æÎ×?È}+å6%+UNASNone?ï›W êŠ'?ˆ~Ï0,Ø ?‰*֋g}?ˆ~Ï0,Ø ?ïƒt^v­Ü?"ú—)_œ^?"èbTˆî?"ú—)_œ^?ïPmÈV?ŠÃZ<¤?•òFøÅ Ÿ?ŠÃZ<¤?ï¦,|µ³+?iÕPd~}1?†tàÖÑM?iÕPd~}1?í"z¬õ†?³i Ru?³\+ƒGQ?³i Ru?ë똃³Ã?Ãлñeç?ÃàQñ0ô?Ãлñeç?é]‡ác?´òW×ʅ4?ʉáøzr?´òW×ʅ4?ëõþâ+?¦ýá>Á?À(ŒwƒU?¦ýá>ÁAGN4FGL J1338.0-4159¿Ü"R@4
šÃeDþÀ;
ÔoX}À<‡µ¡7Í@  ÍâK ?ú²?'ÌÎz?ÕòÄMã
?Ò¥kŸ`X@(‡€'a—@Ç°-YÕ¿ïöÊÍL'?횣"Ôæw?֓åDè½C¿ß5î#‰œ÷¿ÍK€†ù¿éÒ%œq».UNASNone?ïþˁ7ý?%MÛE¾?#Gê×"0ï?%MÛE¾?ïëöа?pv¼"²µ?dú	ô.c?pv¼"²µ?ï݆p…»?kX"6.(?q<Çænîz?kX"6.(?ïü™¤^ø?'³Ø{òM)?;2Üü'AH?'³Ø{òM)?ïþû-æ˯?þM¶? M ðŠÂ4?þM¶?ï‡*þÓ§?˜Nø3ùnÑ?Ž5@@ÇLY?˜Nø3ùnÑ?ïÙ¾,¯?wZ­zhþ$?s ÷ö¶ö
?wZ­zhþ$?ïøE®àӕ?CÏ
)Ҟâ?NéEY²$Ç?CÏ
)ҞâAGN4FGL J1338.8-4509¿éóÂ"µó©@0çm"BJ'À:·)Æ¢ç À<6,ém"@MCtôɖ@ËHûòTF?Âü¼Z
è?pý
~Êeˆ?²y=®ŒDò?øà‹ÓÞ9?̙ŽŒ"Ž?éêô€­¿ç

Ÿû³j¿å¨šÞ"Ô¿æ60ÞÅÕ¿µ8äx0JUNASNone?ïúxMt?AUâNƒ	¤?GºBÖî?AUâNƒ	¤?ï½½÷á'F?Šÿ˜q¾mÀ?€',©?Šÿ˜q¾mÀ?ïä	v¹x?jY)µY?köó­wj?jY)µY?ïÂk'Hp?dBê	mlã?~Êp3ì,?dBê	mlã?ïêz*ß?b™Àœñõr?e…bõˆË?b™Àœñõr?Éõ¾?³<•=C¡M?¦•ó\X›x?³<•=C¡M?ïÏø¹˜E9?}•©ÝÏø}?x£Bû«D?}•©ÝÏø}?îdî#+¶?•úÅÉòS¤?©±ʺO§?•úÅÉòS¤AGN4FGL J1343.5-6827?dÜEÀHŒ°/À:ËCæÝõÀ<,Mâ"s@=;"@óÅ¢6 M?×*Ÿ[$"Þ?îÍ~d^N@f"»ë@;(ðÁ?íÛûß	s¿ÖAcAî·Ù¿ä(³GÀˆò¿ï춬Ï×C¿Æ¹Ä1r¿¿ïá½õ™t±UNASNone?î)ï|#?´É²ï‰˜Î?­oá
œVÕ?´É²ï‰˜Î?éhÒí"WÄ?Åô?Ói?Ê\´Kv ñ?Åô?Ói?ë	T§nÏ?ª¯îZ;4ß?ÃÚ­bE¼Å?ª¯îZ;4ß?ìæUJùè?¤ß
Ý»"?¸ÏEVò=?¤ß
Ý»"?èÜHcd?Ë[
"!Â?̎ßûÂrp?Ë[
"!Â?Æ^*äm—?Ê>iGA]?êhu{Æäš?Ê>iGA]?ߐÙ.ãuä?¿óºÑ'qq?à7"hŽE?¿óºÑ'qq?֐ꪾÊ?ÈPØ4´è€?䷊ÿ* ›?ÈPØ4´è€MIXED4FGL J1345.9-2612¿êŠ-ZM ¿@A‰:'£SÀ:¹Y×êðÀ=£.mѕ@©t$j¡@Ç<t$•?ȋË:PˆÚ?ïþƒ~$H4@&\âY&@	>èŸf7B?íPŠ\õ¿ÚrÃ×ZÅH¿©–Ú]À5Ì¿él«úÅ-œ¿ïÿþøþ"?ïj8$óTUNASNone3FGL J1346.2-2608?Îóژ<wU?ÐSÞ®Œ)?èC	Yðâ+?ÐSÞ®Œ)?Ý:ÃüªÇ%?ݞ¯ê$2?ábžªœn?ݞ¯ê$2?Ù]ޙ?š?µ@£™ƒ¼f?ãQ³xà3?µ@£™ƒ¼f?ÝÒ͵Þ|U?¹VË«Éù²?á™%ÁÕ?¹VË«Éù²?Ú{2ËÚ3"?Ûf.Ñ,`?âÂfšæ7?Ûf.Ñ,`?µ$¿ŠS‡e?·5Ž-œô­?í[hÃMƒ?·5Ž-œô­?ѝ͌KŽ…?´N¼ Ò?ç19Ú8¾?´N¼ Ò?©é¨ÜŸ×
? …ª™.*Y?îaerlüO? …ª™.*YPSR4FGL J1346.5+5330?рUw£@NÜz¿¹¾ÓÀ:h™î˜ÏÀ<ž))Äõh@œ³ì+6å@ö"ï¾i?½–Öñ"×?¹6w‹QØ:?÷W›ÈH@§¡§…§?êà^úâ4¿æËÔHµ{¿é€NÚX¦Š¿ç!ßeUÅ¿ïù¼º0¿Ù&ðކßUNASNone?ï÷à#–³
?Hûžõÿ?P?¸xýµd?Hûžõÿ?ïÜâêz?vÅñõþÛ?qŽŠÐ[«*?vÅñõþÛ?ïÕ+Śm?s˜¢êj?uvj4	n?s˜¢êj?ïO'§Ã0Ÿ?€—ø'nJ?–«ÁV
?€—ø'nJ?ïæ{ ›|¯?dRÝLÀ°±?i"_ üpÉ?dRÝLÀ°±?ïET—F?Ÿí¶HÉ??—U|GôíE?Ÿí¶HÉ??ïÉ	Ã<%?~ßùÍ{fZ?{{@÷-×?~ßùÍ{fZ?êà³æe¾å?®j2k­?Ä}0fij?®j2k­AGN4FGL J1348.5-8700¿áh«©ÒÀ8;*'ñ¶'À:ˆ cLÖrÀ<2
˜à66@ô%8Kv@Ô¼÷"?ì˜ôX,¿½­‰:¦Äû?Þd¸[¦™Ý@	D&{Ÿ^?Ñ''?X¿ãáÚ{9¿í^lœáL·¿ïþÂþ—Ë
?ïñhÃ7ø•¿ïÿ'ö֌UNASNone?ïôÚešA=?žíJ›¯ži?VK4]ŠÅ?žíJ›¯ži?ïöSUȬ?X
Þƒ?SYÅYî^?X
Þƒ?ï&K}E¿Â?—¡ìJˆ??›6R Õ?—¡ìJˆ??ïÿøþPtÚ>ÎUk>;‹¼>Ì"¬Ð½Ý>ÎUk>;‹¼?ïüRÏàe?T~Ôð%x%?=i‰YÑÈ?T~Ôð%x%?ïÚvÑm›d?} 5ðH–?rė,U–.?} 5ðH–?ïoG²z?™@[P7ï¾?œ²½èè¾?™@[P7ï¾?ïÿ&l.(?#ßÏ};?2r½ˆÁ?#ßÏ};AGN4FGL J1349.1-5829¿ê'Ä5N–f@Rºû15À9'ðrÄB»À;TkJѵ@ÇÏÿZã@ù†üÞãP?ÇSÖö·W?½0Ãj¥?ö"fÿéYË?ûr—w*ƒâ?ïÿûÎBÓ¿àxŽ¡îÒ±¿éñ×HPѪ¿éނö ¿Þòb+‰ò¿ïš¢ãÅ6ÖUNASNone3FGL J1348.5-5833?ïó·‡Á*?W(>š:ði?XðÒâLÓ?W(>š:ði?îŸÓöÈÚá?¬3óxÏ?¦À•*î?¬3óxÏ?ï^Hió†?ˆC95ŒÆü?"6òÊ&C%?ˆC95ŒÆü?ïAó¥Ø?|ÆÔá©]É?—ß‹Nù?|ÆÔá©]É?ïÆj-×dç?}ɗ®rò£?|Êé!\5?}ɗ®rò£?äC×R.B€?Î}6ƒõ˜?×xQ[£{?Î}6ƒõ˜?í:
Î÷/³?¤!ø•€ïÏ?¶/©ŠlCå?¤!ø•€ïÏ?çºí7*
?·£"tž?Њ%'ù«í?·£"tžAGN4FGL J1350.9-2757¿Í÷[¹¼û@@ŒÜY1ÊÀ:z(4Òo¤À<Ç]!CG@ÌÆHy@‰@¢\›âI6?Í{±ýºÃ?Ðé̂$2@;#Â|è?þ9—ÒÅ¿îðŠ!«¢?ïDŠ=Ü¡¿ç®ùþY¿á)-÷¿îk½Þrf¥¿ïìœ
!¼UNASNone3FGL J1351.1-2743?ïÏÀ"|œ?…íÁ'ìÇÙ?‹ÌВ$?…íÁ'ìÇÙ?ì³þÛÎÙ~?¶].槧??º`	!‰4?¶].槧??î›r÷½?•3¹LP³?¦HЊcÊ?•3¹LP³?íh×k•?"ãDv-?´¹C]@Ü?"ãDv-?í,
¥1?°®›allë?·Ÿ'Žû?°®›allë?áÝU®æ»i?ÑÄ`]žýÃ?ÜET¢2‰.?ÑÄ`]žýÃ?çs'Š£ p?´˜çÌeEj?Ñú깿 ?´˜çÌeEj?ÜO:óÓ?½€™XG#?áØwb¸?½€™XG#MIXED4FGL J1351.6-6142¿àԆ°fmP?ÕÃí_êKcÀ7þ§vÑîuÀ9òzƒSÜ÷@Î$ªYZ@(H¾µ²Õ?¶>$'ýu?Ñا¡o%þ@ƒ(ùôMD@n,"Þsé?ì›Æ/#Ùú¿¯¦^B¼¤¿äÛé B*G¿èõ~ò¤M¿í3nŒ¥•P¿ïÿúVrÓ\UNASNone?ÌÈß~¢•?Ð>Ø®¤»?èÍý W[?Ð>Ø®¤»?¶¾cÊ͵?°8åë'ñÆ?í(3†¦^	?°8åë'ñÆ?ÊÒRc¶D?³£†Á?éKkgnÿ?³£†Á?·ð½?ę«?£E%G9ë?íèW´›?£E%G9ë?ˆÙà"Qq'?·#gš5NU?} ûÊ?·#gš5NU?'¹?Ó/ây?…Ø"?&?ïµr§Î?…Ø"?&?ŸëâN¯´?•žmâÞ;r?ï íSˆœ?•žmâÞ;r?RÝ&Ñ@õø?GòºríÅì?ïö'l×ø-?GòºríÅìPSR4FGL J1353.5-6128¿çˆrn¡7?à´¬Ã˜À9­ê‰v6À:DmŒËU@ !€
+Œ¡@Ù\T"­?ÑÜ©ò­1?Ð¥·_'WÞ@–ѵ(k@_ƒmÞ)ì?ïQ½ei¿Ù¬bÉù³¶¿æÍØÀË◿稊-¿ìèÜy¿ès¥J_ UNASNone?äÚ7Ý£?ÑXNµ¼?ÖKD¹Ëò?ÑXNµ¼?êM'ÎP/˜?ÃþeÌ³m?ÆË`Æ¿AŸ?ÃþeÌ³m?ã¼u鳄Ê?¶ç%­Àk`?؇,˜öm?¶ç%­Àk`?ë '°¸´?§Ÿ‰džæ?õ}õ=1?§Ÿ‰džæ?á"ӝ\®?Ï'¹9iz?ÝøÖXÅF¤?Ï'¹9iz?×.ÃP»óû?ÑaŘÈ?ähžW¢?ÑaŘÈ?×ÈÓp!rŽ?ºFŸOíº?ä–GïF¹?ºFŸOíº?Î'à¼\·?¶Ñü¥Ú$?èvÐü(Ò?¶Ñü¥Ú$MIXED4FGL J1354.2+0353?çvr¼ÏÃ@O,*^x[[À;]ôiÉÈ6À<®$´ë.¸@ ͇‹z&?ÿÄXŠÑ?È[XjËP¿†¥VøE‡°?ÀÎ2èà~°@9ÂÌÓ?ïðp
TÙ¿æo^݆Ž¿âWʌ€¬c¿ìI!ñ¿Ë?ÔÉÛÁ‡I¿Á•ãšzUNASNone?ïá®´ïò}?ª_¿>þ¤?nQKËòü?ª_¿>þ¤?ïñÐ2Ä¿?còڛt?\_š‹,Q–?còڛt?ïÇ°²~±¦?ÅH(u°?|'¦žKc?ÅH(u°?ïþÿO‰ˆ³?ûZ2? 1ïV‡?ûZ2?ïûàr_Ý¥?CSi2:9?@~7@ó‹	?CSi2:9?ï¾g"	Pr?ŽÊhjÞ²?€f7†òÕw?ŽÊhjÞ²?ïÆ$ª.gG?"ÝŒz±¨Ø?|íª÷:¸¦?"ÝŒz±¨Ø?ïøew'?LQ•áE0?NkŔû£?LQ•áE0AGN4FGL J1356.0-6747?Û«PÅUÀÄSK×nçÀ:RebZh+À;Â)©FµÇ@¦¿Ë1—'@¼¬ùÈ®Z?Óˬ¦¼—Ë?è-3¿Ë¤@yl$ìH"?û[9i®ƒ?ïFòbˆ‹T¿Ý½<‹÷p¿ëXd"¿íÁED­®ú¿ï¼~Æ.£¿é—€ŸÍAUNASNone?è.J÷Rºì?ËMי"uñ?ÏFÔ"µR?ËMי"uñ?àòÓ¼Ö	·?Ìíö±*bˆ?ÞX†Sì'?Ìíö±*bˆ?êÏ\oÓ³­?ªxWƺ?ÄŽ@±1L?ªxWƺ?â¯.×-ú?±=~Ï̃?Ûö¡¢Q¤
?±=~Ï̃?Û+û9$lz?Ín¢R®VH?âjcmÉÃ?Ín¢R®VH?·€ò_!s?Â9$û\Ð?íá½}W!?Â9$û\Ð?Üÿè`¯¡?ºS»d?áÀϨ0?ºS»d?¨Ûªºm—?"‰š­q»û?îrETç?"‰š­q»ûMIXED4FGL J1356.6+0234?Û4+M-'@Nt*€JÀ;ÂÀð À<Úü›ÇqC@úk­ø÷"@ë=Ñ?ÐmÝvV?éºÅ˜ûäè@ô]…TÖ@ûlYA:¿åÝlÇ©w¿Û É8Õì¿Ç8ÖöœT	¿éŸxÁ1ãþ¿ïÿÿ" 5•?îƒÁ@&¶£UNASNone?í#‰ÛÇ¢¨?¿,LŠÙH—?¶ã±"0ÞC?¿,LŠÙH—?ëãªMµ¯?Ä*Z°?ÌqVÉ)C?Ä*Z°?äOX²–>?³™GV"/Ë?×aNšÓç"?³™GV"/Ë?íFÿòzA¡?¡[t©væ¤?µÈk¿ÿz?¡[t©væ¤?àØïKìb?ÒjGõ•¡p?ÞN!h&ý<?ÒjGõ•¡p?ÔÇ£îX_?Й|Sô¯ü?åœ.üÓÑ?Й|Sô¯ü?КÒ/H~/?·ç'&t0?粖è[Àè?·ç'&t0?Ü.…
	lª?ÁŠ¹?áè½y{I«?ÁŠ¹MIXED4FGL J1357.3-6123¿î»¯ÀÄÎ?ސpõ³ À8ïåÍNÓÀ:æ	´´¨@7‰Ia@ŠR¹á7¾?ËÛ)†âñ?ß[_!M­ˆ@þª°BR‹?ÿžwì©·¿á$rÀç¼<¿¨}ô]ƕâ¿ÖÝË!Ñáà¿ë·†Ÿ@øn¿îÿãIœV¿èD?JÑUNASNone?å?y"¸Ö˜?ÔY|G'?Ձ֎RÐ?ÔY|G'?χíÈx‡Ú?Ş°¤øóF?èáÞ
?Ş°¤øóF?Ûv±–Õ2ç?¶£Ï¬¿ÕÝ?âD§4•f?¶£Ï¬¿ÕÝ?Ù¶' w¼?µ,eÑ¥?ã$ìoÄ!ò?µ,eÑ¥?À±‡ARZÁ?Å6ÊcÞC9?ëӞ/«iP?Å6ÊcÞC9?ÜeÈ"ã?—…@â—f?ïy×&B	?—…@â—f?°¨(&Ž•?ÜË!ÅÛ?íêúûtn?ÜË!ÅÛ?‹Çҋ)sª?~¨¯Î²E?ïàµ·ÝQ?~¨¯Î²EMIXED4FGL J1357.9-4907?ït¯ÿ®î¸@(¡™V}»À:ÜþÒ—À<¨Ï—'h@¬Æã#@¿Åäë?ÅÓ\ÉY¥¹¿ >ªhR?݊´cõGë@z²ái<?ïÿ< A¿¿æ…¢×/ý¿ì·¬ª–¿µM`:—¿è*øÒU-¿Þû¶YÃÀµUNASNone?ïúˆït¹Þ?Eœ …B¤K?EÜC £>o?Eœ …B¤K?ïÞÁò,‹?xã$ÌÃà'?pŸqå=Žƒ?xã$ÌÃà'?ïƂÝâÁ"?€3R0…/?|¾'`^ë?€3R0…/?ï÷_I*…)?7+œ)ä?QAm'¯?7+œ)ä?ïܓ)pšO?w@¬k(?q¶k,5øf?w@¬k(?ïñ"‰<Þ?¨GU¼?œÍ –L?¨GU¼?ïbtòÎǬ?'*À´?"±a¦'
u?'*À´?ï¿ýªvqÝ?q*.Uì"B?€•Sõ,¶?q*.Uì"BAGN4FGL J1358.0-7749?Ì	°7À¶"À.Ök\šÀ:{@¶©tÙÀ<)ŸY@J›÷lÞ{@̳_=}9?Ìu´øo½Ó?Ç{V¢ùê'?üû=ÈK^?ø))ò—·—¿ÄÏ8
û¿âs~&÷f¿ç©>RK&¿åãHÿù¿çú¢'ݔ›¿ïÿ/‹_UNASNone?ïï/ò¥¾/?Xªc] Ù¥?`Ð
]˜ã?Xªc] Ù¥?ïpO¬Ì¸f?–+îÈqµ?'ö
d±%??–+îÈqµ?ï¤àÖUGì?'hEH:£?†ÇÊxltß?'hEH:£?ïN.÷»¹?u¤TùOa?–:?:)Pï?u¤TùOa?ïËf%"ú+?v§8q>9?zLíWÕ~ ?v§8q>9?ì¤b?'•—4<?¿Ï7úÜïI?'•—4<?íOº—.õ?§–Œ!u–f?³õ'*ؔÙ?§–Œ!u–f?é\ù¢0?±ýBF²¨?ËþŒu¿A?±ýBF²¨AGN4FGL J1358.3-6026¿ïã6¯z½?õƖ^¤ÑÀ8"n°'-À:d>XˆW@x=û»ù@‰¤Y=?±XR&"g¦?ÑyYˆ1'@@@&`½?ÿF
ñ/W±?îöø_LÁ¥¿Óîtý­ë5¿ãKíÿ¢b¿èÉf@¿ëÓß ¹ôX¿é3€`°UNASNone3FGL J1358.5-6025?³oøï1?ÀY(í½'?íò¸âŠ?ÀY(í½'?¶‹¬n©?°'†wR§?í.Š|›1?°'†wR§?˶Ô?³ñÞ§†:n?é~Šýýû?³ñÞ§†:n?´NTʐ:(?›d…'×q?ív5fò°ë?›d…'×q?k žOœ¯}?'‡öâ}–·?ïä_aÔ@?'‡öâ}–·?'†¹ÿ}ìš?"ù1›̶?ïµåh&?"ù1›̶?‹œÅ$g)?Îù½­®?ëòh#?Îù½­®?S(s"_"?Eïó&?ïökÆfp?Eïó&PSR4FGL J1359.5-6615¿Ñ;9«·HÀ&0"ÝzšÀ:wŒ 4RîÀ;¤»5˔@Hàø'ï]@yYE³Æ?ÆÅÒG5Ä¿¼·^""m?¸ßw^Ü.j@ú\­U
N?ïôÊ(,o¿æР@ý¡+¿æ'³áÄU°¿æWæ`ǖ¿ËTO£uœ¿ï¤œ—zÛhUNASNone?ïøOÆւr?BcGd óŒ?NÀäú\?BcGd óŒ?ïç'Lv®¼?u¢ÆÖ¸¼?hn³ºË¤?u¢ÆÖ¸¼?ïĪd œ ?{M…l'‰"?}ªÍ·A?{M…l'‰"?ïù(‡!‹°?4lµ¡_sj?K]ã3rÛ?4lµ¡_sj?ïåÅW@6Z?bý4xt‡D?j:¨ô¶,?bý4xt‡D?ïqß"1P?¤ô³ß§·?'ݤ¹Ö?¤ô³ß§·?ï=ß±Mb?"5HÔ]¤q?˜\D	ÖSÅ?"5HÔ]¤q?ïË´Æ¢3?oö<ÆN•O?z%ò­ÜòŠ?oö<ÆN•OAGN4FGL J1359.9+3616?îÖRpÿá;@R5!…Æ~À:¦ªWVþêÀ<"웟-W@+èJ%@§†
¢?ÃٚæuÀL?¬jÐa	Ñ?â%ëoOC@"N0"Þ¿â¹_'F–½¿ã¨"ÿÔò¿êÀÚPC¿ïØ]ÂRö¿î媞ú'¿Ü¿³O÷9UNASNone?ïúÔÑ%?J£{2Ã?G€°Ë;C/?J£{2Ã?ïá`ìe)·?€_"_?nŸi[é¬?€_"_?ï©#2ñ*5?÷±á?…·3Qsâ'?÷±á?ï¥@†­Ù˜?só–rð"í?†¯ÞWù6?só–rð"í?ï䖈u¸q?q¤Åz¨§¦?kiwŽg|?q¤Åz¨§¦?ïYež·³?¤giZ\y?"ÓL'QÑÐ?¤giZ\y?ï‰ù[åÉ?‰úRyÇ·?¼Až·¹á?‰úRyÇ·?ì'lÒ¶"?©ÑO'×—?»lŸ)jKg?©ÑO'×—AGN4FGL J1400.0-2415¿ÕQÌ—Â@Bt§qÉqÀ:B¿ö$´ëÀ<}+é'Ö1@%Ù}_QI?ûÎ:Ufcâ?ÃÝýâŽl?ß(Cëè@fX`f@ŒÀ0Ýž?\X¿Ô¡—Zû¿Æ.·ùVº¿ã[ãU¥N¿í€<›'Á^¿ïË!6±mUNASNone3FGL J1400.2-2413?´ô²Ï2ž?½/B&¯Ûê?í!i˜[<?½/B&¯Ûê?ÖÎ9B…¥`?ÆÊòÀZZ?ä˜ã^½-P?ÆÊòÀZZ?Ê0^äG?®†[ï×ù-?ésèzÛÆî?®†[ï×ù-?ß:îޚž?²•VkÔ?àbˆ²À1?²•VkÔ?—8¯sQ¼?²¹úr®?ïF:ƒMk²?²¹úr®?´m¸±*?µ9~ëõ/b?írH闢?µ9~ëõ/b?¢C+¦[zÎ?"ÙŽkŸ?îÛÍEã?"ÙŽkŸ?¶(š²Ä? ›j	v/ä?í:ì©Ð¸.? ›j	v/äPSR4FGL J1400.4-6050¿ï2IÀcL?ìóŔÊ'À9·ÓôzùÀ;CÓÀí@l§"W`9@΍F¤ÿÿ?Ѷùü°À'?æ†\㔏@wàmò@ÜòJµ°Ñ¿å>, òÔH¿æ¨!â}ä¿Ñ}Ýï<¿å.	"&¸Ñ¿ïÿý`éNä¿à–
~C›UNASNone?⋶ƒ£ýº?Ì÷.žº?Úè'ø¸‹?Ì÷.žº?땁ʣ…^?¼¶Üàû¿?Á©øÕqê‡?¼¶Üàû¿?åû,QuF1?±WքˆDÅ?Ô	§]sž?±WքˆDÅ?ìú1uh?¢WM-ý?¿ .wüT¿?¢WM-ý?Ök>AÚ
?ËD ò¥	Ë?äÊ`ßõ{?ËD ò¥	Ë?ÓÓ֍&)ñ?ͤD寔$?æ¹lë?ͤD寔$?Ì­¥õÈn™?¶i­å‹G?èԖ'äZ?¶i­å‹G?Ø
Åp–?º™…oŸ˜?ãÿzðGµ?º™…oŸ˜MIXED4FGL J1401.2-6116¿ïZÀETóÍ?ÞQ%ʟÀ9[(5©/9À:Ób¢Œ‡b@·:ööìÜ@ª`üšò?ʗð!:¸8?Ù¿E» '@
	_à:gÛ?övàœià¿íD]Ä×5?¾æ]Â}ée¿Õ˃ÁÁ¿âÎòJ¶Ý¿ïDá±``?£Œ'ìG-UNASNone?ãé0kˆ?Íq͏aÔ©?Ø-žß(Äð?Íq͏aÔ©?ØԞʨR?Ìg_ñ¾Yÿ?ãñ•°š«×?Ìg_ñ¾Yÿ?âX¶XÙ?µ—¦X‹?ÚáN"OÂO?µ—¦X‹?à6¢+8'ï?µßIæ£Äˆ?ߒ»©ŽÚ#?µßIæ£Äˆ?Æuæ6*^?Ä%»®õÔá?ê~â†ruh?Ä%»®õÔá?œÖìä®æ"?¨è˵1ú?ïH˜ö«?¨è˵1ú?LJYÑ»?³´qT?ê8)‹¿'?³´qT?ží䫂þŒ?!Dáù?ïÚz¬¼?!DáùMIXED4FGL J1401.3-5012?ïëO¿äd¢@&Aòý¸ýãÀ:SQ÷GËÀ;åF­czú@1ʨZR@vÜB‹•Ë?ÉŸY¢Ò?ÃsÇ¢ìS¦?öO²$ªÚ4@›±vÚþ¿â¡{_ò®ß?ïõ–Ÿê³¿æ¿a>ß8à¿ä¾É¿Q9.¿ì¥Xtá¿ðUNASNone?ïÏãчWß?wmp½Í–y?xGRЌ?wmp½Í–y?ïcŒb?›Ñ¾¥Ìëœ?"œNƒ/o»?›Ñ¾¥Ìëœ?ï8½W¨¢:?Ÿu0·ñ?˜èU"»?Ÿu0·ñ?ï'S¦è"?r&EÂâ}?kINšÆ?r&EÂâ}?î¼6 Å¿µ?¡¹ëU›_d?¤<ñì6¸?¡¹ëU›_d?ëk€µ$Ã?Ä®÷žKsá?ÁÂQý+lô?Ä®÷žKsá?ì/h¸Œ_?ªˆóÅdB?¾‡Dº;?ªˆóÅdB?캱$?©:L}Ã5†?¿/Òwþâ?©:L}Ã5†AGN4FGL J1401.6-4645?ÝÑt!N@,×`Ï‰@À:_!©ó›À<Á±æ—y@×\Q9®w@æ¤ì´?½x؃å'b¿±=Þ^p?ó{;	ÁIâ@·•‡U
¿¥ò¨ êé¿é
á,ˆ¿é//˜sÿ¬¿àC݊¿ë$®ÖAÀ•¿¦&™áÔpUNASNone?ïñ°?#š?Yt˜FÊø?\Ÿ'A±KÍ?Yt˜FÊø?ïÝáûGÈ?z"¢ö̽?q\È7?z"¢ö̽?ïÚ·G:¸I?pé\¢²ºÚ?r¤\fÃc"?pé\¢²ºÚ?ïööðƒ"?8ì>Cüx'?RvÄ«·?8ì>Cüx'?缾äÕ?"O·s'WU?…S¾)¥?"O·s'WU?ï]…—./?¦{äîOÖ?ÔOKbl?¦{äîOÖ?ï'Y]X9—?Œ~]Ë?‹i¨œ3*c?Œ~]Ë?†"œ?yé‹f›Í?ˆÝžQl?yé‹f›ÍAGN4FGL J1401.7-3217?ét§L4¶ì@<EB€®IÀ:½–V;À<x¸Œ£è@WrÜÁb?ýTyð'Î?Õó!à¥q¿?ÖÂhż7S?û\ߺZç@QG9Oó?ïyn‡P¿çl…>õ!¿âãÊ|"¿ØŠYàœ'¿è¬¦Q8ø¿ìžÑÿUNASNone?ïû樓8?@!†ËÞ'?CèA¦+L?@!†ËÞ'?ïò)/Eµ8?_?6:ë^–?[­¡í‡Î²?_?6:ë^–?ïÁúAWÂ?{¹U}á.?7'èC?{¹U}á.?ï÷R'GË#?4Áê¿?«?Q[±Omyt?4Áê¿?«?ïùÕÆy)?NF6֍ä,?Kü©j™?NF6֍ä,?ïȝAº?€"¤áSM?{±~b'Ž'?€"¤áSM?ï§ÌÁÓä2?‡xà¼mÙø?†ϑæ+t?‡xà¼mÙø?ïêáãèÐÂ?R,ÊÐQž?e.Œ•Ý?R,ÊÐQžAGN4FGL J1403.5-6236¿ïØE«bw¿ìD¤¿èbÕÀ9NûH
[À;ži9}@ŠÊ"£n@í÷­K'?ņIÖ©?ï›ü€¿@Žï¬.@ËÔ²IhÕ¿ïÿÝ/ñ_S?ïÿp\‰¿Â©•e,¿ã¼ì™.:¿ïÄaùð†?½•æܘqÑUNASNone?¬*œûg®ª?»	Iþѓ?î=V0I…?»	Iþѓ?½×…ÁK?µÞ¦þïÐ+?ì]ůG×?µÞ¦þïÐ+?ÎF÷^#j?°j:œ¹(?ènB(w &?°j:œ¹(?¶ì¼¨œª?£J]ÌWë?í"~h¡æ*?£J]ÌWë?sBšçDð¼?¤!;>8'¥?ïÙzÊmï>?¤!;>8'¥?"Ýüug?†¯?`L¢Ä?﬈+çº?†¯?`L¢Ä?´}á%ä?¤PU]ù‡?ípCۈ7®?¤PU]ù‡?h,Ö¸º ?X娠c¯?ïçÓ)÷äí?X娠c¯PSR4FGL J1403.7+1513?Ñê#¨YX"@QZ0#̎À;hÙQ?µÀ< cÞÌ©'@A_ˆhš@–•3®?ÌOÈ?—Á"¤+1Ì?̒ ¾ç[ï?üŠQՃ¿ïÿÿ" 5•?ïÿúVrÓ\¿ç' ¤:\¿ãUGá‰ó¿Í–õåÊʔ¿ïÿ%¿Ø·UNASNone?ïô!D?ÂZ?i|¶øºz?W½wx<;Â?i|¶øºz?ï֗®ÝÎ}?"D˜ÇrÖó?t´(•8I'?"D˜ÇrÖó?îÔÉfÌùÔ?™SÝÖ="?¢³iœ­¼?™SÝÖ="?ïß>¼PÂ?]tߝͻ?p`üHzË?]tߝͻ?ïî'ˆZÏ?xª~Áß?a}ï­?e?xª~Áß?ïÞ¼ÁðX?¯#zé·0‡?ŸD(n¡,è?¯#zé·0‡?îÚ¶aüIg?› h@¶Gˆ?¢T™áó7‹?› h@¶Gˆ?ïït}¼€?"OÒ9îð*?Ÿ'ii8?"OÒ9îð*AGN4FGL J1404.8-5237?ïáçOž½Š@!M¤¬ó²À:lÚ"À;癴qŒ4@NMlDvÒ@ˆ¢ù"«ô?Á6F8¨²?Е§œ'›ž@	ŸNÒö@+Å ¿Ë,a‡ÚTu¿ç¼"pdìê¿Ôïʓ6©	¿æÖÜH¿êþz#²Œ°¿ðUNASNone3FGL J1404.3-5241?ë"O•ï?¼ÜÔy5îF?ÁîÁ«ÓÐD?¼ÜÔy5îF?í»Û¶¨%×?¯M;Îáo´?²!"K,ÄÇ?¯M;Îáo´?íŸå˜B#? å×°Œ—?³Ó?¦µÁ? å×°Œ—?î®r³j•?"KNÁ±Ì"?¨×]®?"KNÁ±Ì"?Ý÷5¹þÇy?ȖO•Èr?áe#œC?ȖO•Èr?àLŧ$ع?Ïý¨6È?ßft±¶N?Ïý¨6È?àÓù·f‰!?»€h}jô?ÞX'2í¾?»€h}jô?å[2çÅ?³P˜ ð%ò?ÕÿIš0uò?³P˜ ð%òMIXED4FGL J1405.1-6119¿é¡ÑdÈ<Ö?Ò&Ÿ;š
À7€®I#À9iÞÎW@	¿Bu›c@PŠ"Ràx?±M
NóA?Ñ(6À[zO@"µz»ˆ?öŒ¯˜ß_w?·Ë¼V‡÷¿×ˆï]J¿æ«"zuè¿éç.þL²¿ë'®/RÓâ¿åï@4£UNASNone3FGL J1405.4-6119?Š'îiQ=º?ªmò*'?ï—`F'´É?ªmò*'?¯þ²Û±'t?¨_) ÙÁ?îÒ
î?¨_) ÙÁ?ϱ\#Ax›?¶gdw<¼8?è¨÷/¡Ù?¶gdw<¼8?qGŸ·üí?cäÙ>»I?ïÝÅpÀ?cäÙ>»I?x0fn?­9äBÙE?ïϟÍ1Ãê?­9äBÙE?€ìyÜ·[?'áuýáÙ?ï¼Nä.‹?'áuýáÙ?¯#ï,úÞ#?£ùœã?î
Á
Õ>?£ùœã>éŒCLô‹>æó­°0ux?ïÿæsÖ«7>æó­°0uxPSR4FGL J1405.3-6008¿áoóÚû<?ö«#/¯ñÀ:4äR´ÙÀ;^¤€}há@!¹ÙNehº?ÿ7½¯lj?ϧWGd˜†?³TÐùøT?åóÕº²@ò^ªuÛ?ì‹m¡Ä
†¿ënÁê»m¿æìma,j¿å!Á›Á<¿ÜˆC{)ìã¿ß]©~i'UNASNone?ïý¯6wƒ?Bo.Ú[4?2‡ÅÔk$i?Bo.Ú[4?ïÝ·)ŠØ?sap»-ƒ?q$1gÊø3?sap»-ƒ?ïӓn˜u=?{8°6pTÔ?v6HË"¹ ?{8°6pTÔ?ï÷{—0D?=@É-	ë=?Q	Á4"7?=@É-	ë=?ïüñg?8Ìý-ùNq?8wÞøå)É?8Ìý-ùNq?îç,'·eC?°éZDٞ£?¡=€>(Û?°éZDٞ£?ï1œ·*W?–Þ¬Çix¤?™ÌióK7?–Þ¬Çix¤?ïÊ£Åê0?qúÊÒÚ¨?z®tŽœŒO?qúÊÒÚ¨AGN4FGL J1405.9-1853?íêrÂË@DHFà!qÀ;!¦Mà^À<\m¿ <@ Ťö!d?ü;cž5	Í?Ô-ÁÚ*ƒ?Å(ŒDâ?ì%Õ²NœE@êŒÒ‹Óˆ¿â*"Q€ü¿í#¸Œíº¿À'\HÖ2§¿çKýî,￟‹råOпïÿþÞ÷UNASNone?ïòÜ'LŽé? xúœ ¯
?ZG±k? xúœ ¯
?ïó³Tða?\Su·«í?X™Uà?\Su·«í?ïãCúÎ	?k¡*ËCTz?lã¼:ËÞ[?k¡*ËCTz?ïþS6L±ù?#U¦‰Ê_?*̚(˜ˆ³?#U¦‰Ê_?ïý¨"U¯V?38Œ`ü?2»^éW
–?38Œ`ü?ïÉ×É;Y?Mì@1S?{t8?W?Mì@1S?ïͲb4ÊÚ?};Ú·G/º?y&ÎÌÝbú?};Ú·G/º?ïù/nM)?Dœ·eಉ?KCái>%?Dœ·eಉAGN4FGL J1406.2-7500?ïïÚÏç+À)²<êlÀ:§‰i ­ŠÀ<ÖüÑwV@Ðҕäƒ@¾6œt?m?ÈG<)¦íj?¢'­€™l?×VŽ®˜.?ûµ¯¬ÖbM?êŠÍÿ&ç ¿ééH-–;¿àHe)O"£¿ë›—jë0e¿â!iÂ;yS¿ïÿôa¼2¡UNASNone?ïû(zûýE?A?!,mž?C^ŸW¾??A?!,mž?ïÛËh|HÙ?€©Þ:ÔVu?rK§¾‹o?€©Þ:ÔVu?ï³K¿ç??~À<ž<?ƒ-8?àe?~À<ž<?ïâL#D(?SÅé?mð´wÈ?SÅé?ïóHÜ_3?\<ÒX¦Ùú?Y÷n‰i˜?\<ÒX¦Ùú?ïÏÿmo?œ°ÍºHëË?Œ¿õÕÐD?œ°ÍºHëË?ï(bJ«}?"D®t‹ÜÜ?šý3º,L?"D®t‹ÜÜ?îú'h²h?ŽáÛ2ÞR? VïÚPÀx?ŽáÛ2ÞRAGN4FGL J1407.4-0820?ïùI‡L@IÄ"`À:¹Š '§À;¶@­o9t@¦óˆs@W£TY?ÌYAºµs¿£ö傮Ï?̎EèíiÐ?ý 'ç´¿ÔîYyîÙg¿æÄe©¿á€C‡>MC¿î*Ò§a)? ^vÔሿãHû"±UNASNone?ïüÔµ­ˆ?E¡FÄ|?9_Ü|zR?E¡FÄ|?ïèÍƔEê?pÒí¸ÛÄ?g29sù%ã?pÒí¸ÛÄ?é?‡O#v6Ä?žǼ­ö?‡O#v6Ä?ïû¾&c8?3¤>ã  ?Afš³™?3¤>ã  ?ïï%6ñ-Õ?g2Bh?`ÚÈËyÓ8?g2Bh?ïrÄZãPr?:ú•Ÿ?'§tªu)»?:ú•Ÿ?î¯V	Õto?™íèˆÃr?¥
Ÿfô<?™íèˆÃr?ï éáýØÖ?…ÝIJE8Ï?‡Å‡o[¾©?…ÝIJE8ÏAGN4FGL J1407.7-3017?»°5R•@=ÂNY)gÀ:Á°\S½íÀ<"(LOcë@¾t@ꗃ>äA?Îþhö¹…?ë©hyfk@W[_¢'@ûr'¦
?ÅRHw=#L¿Ó?š_<P"¿ãT5â:\¿ïhD¿ïÿÝƒ(i?îœtÀFV¦UNASNone?íWꣳŠ?ÄNÚÝËfŠ?µ@ªã­‰È?ÄNÚÝËfŠ?åN£íc"î?Ìð—Fâ?Õb¸%9º%?Ìð—Fâ?å–Uc×?±k"ª%?ÕâÓU8Qç?±k"ª%?ê h'ö??­€'"â$?Ç~]ô'Ð?­€'"â$?Ý!=÷K?]?Ñ{³à˜‡?áoaZ`Q?Ñ{³à˜‡?¿âº¯¹?ÂßÓìp?쨽½ª	?ÂßÓìp?Öxoõ¨°…?µkÇ§)æ?äÃÈ+§½?µkÇ§)æ?Ãý`Œ÷c"?²õ±Ð"z?ë§ÜÂ'?²õ±Ð"zMIXED4FGL J1408.0+3834¿Þ´B"\@Q"-¶°`À;·¦ a4À=d2‹n@ ²->>T?ü̳¢Y[¼?ӚµUů?¾àŨ]_?î¤âè7Œ?ÿûR[Âsƒ¿ïږ";cƒ?ïõ·!iÝ¿çè§ô¦/ª¿Þ¯¦/OÏ?—øpƒd'À¿ïÿÒ³–šâUNASNone?ïýåÉrû?)›»ZWðÐ?0ѳú3†l?)›»ZWðÐ?ïî™vð2"?k>žF1?afˆå2D"?k>žF1?ïàwFڎ?p¾
ßÂ?oˆþÓBzS?p¾
ßÂ?ïó(r©¯€?Iî	įª?Y¯(Rï?Iî	įª?ïøäéVÎÌ?P0"@7Ç?Ll[$ܤ9?P0"@7Ç?ïµfjSl?™V$N•?'¦ezC@.?™V$N•?ï¸Â©³B7?ƒ–ÙåÕØr?ÏUX<?ƒ–ÙåÕØr?ï­ûǝI8?ÜÑH"Ö´?"Œê?ÜÑH"Ö´AGN4FGL J1408.1-6010¿ÏÿeF<?ô¾C·å´ûÀ9¹™	PášÀ:écyL8@ o+ˆÄà@õþÚf"?Ðli_À?¾"PTVC"?ò^FtŽ@–‰nÔ¿ïùJ¿@ó?îÄgÙ--`?Þ"ZÞGô`¿Þ8_~¿ïû ŠN¢û?ï˜l]vRÃUNASNone?pt\H?šÜõ[X¸ ?‰ÑãæX‰æ?šÜõ[X¸ ?ï€ý½ÛÆ?›¨š6¤6>?ÀÄ×âŠ?›¨š6¤6>?ëËu½O	?¨š5v´†=?ÀÒ)
ÃÛë?¨š5v´†=?ïHÉî~«à?‰H4V†ºé?–æÂ,ºè?‰H4V†ºé?í?¹™>Tú?¹G\óN€f?¶37Å&+?¹G\óN€f?ì*YEqÇ?ÅAÔÿ©Ìu?¾­7õÔqÌ?ÅAÔÿ©Ìu?éAu—B¦?²ìD2ˆ3-?Êú)¢÷Íh?²ìD2ˆ3-?ëBފBY?µeůÂh?Âô…Ö÷¦ž?µeůÂhAGN4FGL J1408.6-2917¿ÞWÑÃV¬_@> í_‹ÎÀ9¯»åüjÀ< ¬Ö(–@$ë,ß1@æ'öÀ?¶õIB¿X?¶[âÿ¿z?÷`ýV"U@]Î_ª¿ÐUýfȌ¿ævA:\ó ¿éÅ(~#qt¿ëp(¡ß¹9¿ã²€áü}¿ïí'ûî£UNASNone3FGL J1408.0-2924?ïùŸíp©?IÅpûF?IƒÌtiã?IÅpûF?ïÆòÓÐ)×?‡ Ž@ÐÈ?|†–%©"_?‡ Ž@ÐÈ?ï{ÃÞø¯?‰‡\¥ÿJÒ?‡""¡Ü?‰‡\¥ÿJÒ?ï¾Ñ2'×?k¤h4³Å!?€K¹(`Šo?k¤h4³Å!?ïàd6`dD?rdï³?o›É¹¸Ä?rdï³?î]»vR ?µ`÷‡M¡$?ª$H™'Ø?µ`÷‡M¡$?ãùd/?œ;š^0O
?¦÷AÃÙY?œ;š^0O
?íC˜@e?§ä¹þhü?µã?>ªÛ?§ä¹þhüAGN4FGL J1408.7-3747?߃}{´^õ@6™Å£ãŸwÀ:˜³"&jÎÀ<`% Jù#@M"òiG@Os²Lï?Êz:°€?ÙqR=9œY@Wކ2´ˆ@$ð"ê¿ïÿû-2h2?ïÿÚÁ,/´¿Ý¢¿³Öh¿åø!ˆ¬6¿ð?ïý¡ñ&UNASNone3FGL J1409.2-3743?æ5'š2,?Ë=?æõÂå?Óõ"Ú˛¨?Ë=?æõÂå?ì]ÑÂTú?Â>ý»F"?¿%qíX3?Â>ý»F"?èåo¿ð4J?­F¢³–q?ÌjA?.Ù?­F¢³–q?¬ºøS?Žç°s'Ù=?¤'50àÞØ?Žç°s'Ù=?ß/袸ž?Ï¡u¦JW?àh®£°¹?Ï¡u¦JW?Ös|Ï^x?Ò
ñwÉ\¢?äýÆA˜PÄ?Ò
ñwÉ\¢?Ò>òÿ'p*?¼žß>>?æà†€7Gë?¼žß>>?åÆI?½\tӚ$?ÕËðsÅõm?½\tӚ$MIXED4FGL J1408.9-5845c?ÐàÛ
9œ@õöº «À9#¹À;íöé@Ê«V™m@Ìhĸ*?Í.rýMž?¬ÛMîöBg?ä£þwiÄ@$ˆJ'Ê?êy]ïŸ_¬¿ä)™A,5¿êI °N½¿éô›Gð¿á)zLÍ8¿Ø'Ü]¹oUNASNone?ïïÚyÄÎ7?bÌKædû¼?`%†\.ç?bÌKædû¼?ï¸^h–'?Ž
ôb…]?èeæØ÷[?Ž
ôb…]?ïß`o£É?"‡õñøð?œî›êÝ?"‡õñøð?ïÜE$;7}?V•"™ƒ?qÝmøaÁ2?V•"™ƒ?ï'\w5?'"ô20B­?hý/ñ(Z?'"ô20B­?í¨\Ü`#è?ºL8xþ³?²½H»<?ºL8xþ³?íŒ#¾ ?¤™ù%Ó÷?³ŸîàWu?¤™ù%Ó÷?îR?A£'?šð¢ïøƒ±?ªÖüv1?šð¢ïøƒ± AGN4FGL J1409.1-6121e¿Ýmî{ÚR-?Àû>û…À6›¾7ÔÀ9!zÈóú8@ «:ðn@(Ôº××Ã?›à¢í€L?¯¼Žç™@Ù¿Š¯?ø¨³‹™Q¿ïÐýH•›?ïðò`Û+¿Ý®êäâ¿âÊâ|azn¿âݹNjÇ¿ãA!"µUNASNone3FGL J1405.4-6119?×)ÉCUÉ?ӄ†X…c?äkrÞU?ӄ†X…c?ÄIR7Ÿ?½™u1…^#?êû-¼ër?½™u1…^#?áàhÎ1§?´­3÷ ­W?Ü?.Äcœ²?´­3÷ ­W?½z8:ÓT?« "KhÉ?ìP¸üØ¥•?« "KhÉ?Ûߤg D¦?Ó¨ÅjÜB?â-Ì/Ý­?Ó¨ÅjÜB?Ýn~É?•ÉŒÝeϧ?Gìþ›?•ÉŒÝeϧ?èSB‡0'Ì?´?¾í?βõã=ôÐ?´?¾í?t#‡ÜÅ?rP€äªƒ´?ï×¹
c~?rP€äªƒ´MIXED4FGL J1410.7+7405¿ìOj¸ýÚX@Dõ*™0¾À:[rðR
À<ojM{³Ö@ ú'WÛß?økŽXó·?Â_Tä³ÉF?Ñ
ƒÁkÔ@€Ò=Oè@ë3zQ¿ïÿïXz?ïþâ^.‰€¿ÒŽä;(u¿ºÅñ;lÌ¿â²€óZ€¿å"ãÓrÙUNASNone3FGL J1410.9+7406?ï`1¡Õ{?""bÀB"?"ùËåDˆˆ?""bÀB"?î»ÍÐÐ4?®'h•è"?¤C"óئá?®'h•è"?íæéEÔJ›? íBtT÷º?°ÈµÓƒl©? íBtT÷º?îË7yœ´?†™]Ú\ʊ?£Lˆc¤/Ä?†™]Ú\ʊ?í±5*•f?®Û¡‹\h?²vVª
ôÞ?®Û¡‹\h?éï€1?Ëî}—Mm?ÈCÝÿ"ã;?Ëî}—Mm?ë|þ
õÀ?¬ð"hŒ@?ÂñÈ)?¬ð"hŒ@?êCv¤n4?±NP^Öê?Æò%nEû.?±NP^ÖêAGN4FGL J1410.7-5945?Ǜ_nœã?ùx"«ËËEÀ9þAˆ`ŒÀ;(šrÝm.@ ¶é—îâ@ît¢iKô?Ç éD&Ëq?˜ÂsªO?ÔãÂwß5@¸áÜò¿ïé|Ñö®?ïól^MW¿çô´±M¿ÞêJa".Ô¿ì	íT+Ñ?¿»P¥	qˆUNASNone?ïÍ°PÏ?‡ö+³¡?y'±mø`a?‡ö+³¡?ïÎbRýË??…Ò_Ò±9à?xÎÖvˌ§?…Ò_Ò±9à?îwCr½Ú
?šòxRÙ?¨‹ÈÖ¶+?šòxRÙ?ïß8RèìN?^(âÞÅ:b?pcÖ«Ö,§?^(âÞÅ:b?îÿ2õö½?žxHµ'I? ÞÝ0ø9?žxHµ'I?îPù0œÄ¶?¶§5÷¼BD?ªðlòÄ£?¶§5÷¼BD?ì‡>îRX'?¨5j«P˜w?»Æm;m?¨5j«P˜w?îìSÄçêÏ?–·Ò!œô?¡:ô	?–·Ò!œôAGN4FGL J1412.1-6631¿ï—ŽÜžž^À™V}»ÂÀ9ˆ̼À<Fí$[@'—îž®¬@UÒ°Y?¼€ìब.?Ùlæ³'à@*
4›èÿ@âd×-©?ä9pÏuôy¿ÓkŠ\å´$¿Ø'Äãõ2r¿â¥,¿ü"˿Wz:Y¿ïÿƒ}ùUUNASNone3FGL J1412.3-6635?¨Ìmñéõy?·æ™º)F?îs9 ï?·æ™º)F?Ø`éÊ^ˆw?Ç´9>KP?ãϋлÅ?Ç´9>KP?ÅgÞwÅ	?®ϳÄÞ?ꦈb¾?®ϳÄÞ?ä61o¹¡L?¬~v¾¯Ò?ד Œ½h?¬~v¾¯Ò?ª€v>Ò?ÂÉmsî0Â?î^§öÝ3?ÂÉmsî0Â?­ôTˆêá?¶¤|ŸÙfÉ?î º·:X/?¶¤|ŸÙfÉ?²8x¡º@?'9l¨âÇ?ïzn<øn?'9l¨âÇ?º¬ø=‹H?ší‡%¥`_?콪`øN—?ší‡%¥`_MIXED4FGL J1412.2-6018?ɔù"]?ð-}|,¡IÀ9δ#ˆ›EÀ:ég•:H@!1د8D@""úÎg×?ÆÕÿ{&¿ˆ¤ÒK«"Ü?Äñê¾zN¦?þ‰×Í0õÁ¿ïÿYø"'?ïþZxòZ%¿çÊ9¿¿H*¿åCÈü]´¿îä£î‡1¸?ç$¯!k4¬UNASNone?ïIJ6ô£?«ýphSx?–ܼ'¨?«ýphSx?ï¯<À>É?"tÅ×e?"0Ïø›®?"tÅ×e?ìDù,.å¤?¨œ±;¶ú?½Ø6žˆÒÞ?¨œ±;¶ú?﷒]» ?t=}fÅ ?'hŠÉø?t=}fÅ ?î'噙¼?±wˆf…3ö?¯
¢öÈE?±wˆf…3ö?í#H6¥ƒˆ?Ãp…üµ?¶å¾L‹±À?Ãp…üµ?ë™ûƒv?¬».€ ?É?јóâ)?¬».€ ?É?í†ô%,?¯?ý;Ž?·sÈ`TÊ?¯?ý;ŽAGN4FGL J1415.2-5550?ífefÙuI@'÷na«À:—J4¹À;hoB­úz@^øÓeî@°;Ñgf?×nA§V?âÓïÖ½@¸®$kT@ÊÂOpU¨?ïë°½¢¿â#NžÉ"C¿ç9Á¢w8Ç¿ìŽÜajS0¿ç‰u"×'ù¿×WÝašy¾UNASNone?ïã\°§t›?rtE',Hë?l£OkÉ4æ?rtE',Hë?í½IÙà(?²ŸÊäÍò?²±/´äÔ?²ŸÊäÍò?î(ÅæY?žbsOžqò?­s¡¡¯h?žbsOžqò?îl_sˆŽ?%›Š˜F?©:WÛ'?%›Š˜F?îó7´ï'Ò?¥Û9î¾X? Ì"­˜6ë?¥Û9î¾X?ڌd5ùOü?ÑD>!½ƒÈ?â¹ÍåX?ÑD>!½ƒÈ?ç{*xyŽa?¸‰NOœ´ý?Ñ	«ã=?¸‰NOœ´ý?ÞáBŸ%¹g?ÀÂU½¥?à^°m#M?ÀÂU½¥MIXED4FGL J1415.3-6110c?Ñå-ÃÔøã?°«ÝSÀ8¡=¼ùðòÀ9àÇÛÌD@ ÄÁ>ND\@ŽŒ:5…ô?÷™»È˜Š¦?ÄNž·Ëß?üG7|n¨@m |ŒÃr¿ë6qY´¿ï;	á€8?æëÂZƒ¿å®²šò_.¿î'lU"°L¿¨k¶B­àµUNASNone?Øâ
?㴊?ԏ'Î?ãŽúà%»?ԏ'Î?ë'ÏÁ'é?Êì$t?¾?Ã`Àûï`\?Êì$t?¾?ÞÜ$$ØM?¶\‹Šý?à'ííüÚ?¶\‹Šý?êõ?öBŀ?·–ËêìÌ?Ä+&ôê?·–ËêìÌ?ϩш{í•?ÒÈ®Ò]Qâ?苝á›?ÒÈ®Ò]Qâ?ãbXµ×E?Ö^ƒÈ:ۍ?Ù;N"Qu?Ö^ƒÈ:ۍ?ÞDÇÒ«Î?·âPy¾S?àÝ·œª?·âPy¾S?Îum•YÃì?ƼîÂYÆ	?èb¤š©?ƼîÂYÆ	1MIXED4FGL J1415.4-6458¿éŸø®R
À]±~'­À:"=n€À<Píè¦G'@®:»gʕ?ýlÇß'Bd?̛ŏÝ?áB!"9Å@Uþ9Vc@hZ‡`%?éHtxwàâ¿å©ÚúŒùx¿¶l=?üoR¿Ô /Jpfš¿êyþ(kB¿çy0m†XUNASNone?í'ªì8‰?µ½9ýiÝ?³t¨ž;·?µ½9ýiÝ?îKI)3‡?ªÃ^o9-O?«KmkÝ+'?ªÃ^o9-O?ëò'ö=ñ?¨ÜV5IkŒ?À5µÀ'>?¨ÜV5IkŒ?í¶W#
²V?dî}\Þ9?²MFç'mM?dî}\Þ9?çP)ÊÃvü?Åû;2Ž¦)?Ñ_¬jy?Åû;2Ž¦)?åy'¼çÁ?ÎÙ•€@"?ÕÛø†0~?ÎÙ•€@"?Ýüh4¶"Ñ?»Ññ[ÄÄ7?áË夽˜?»Ññ[ÄÄ7?åm-ªÞ?²N:}žI?ÕÁ%¤ªD?²N:}žIMIXED4FGL J1415.9-1504¿§(dM1Œ@EŠo½'=\À:ä§0ž-À<€ÇÛÌD@e¸Ž|Z?ûWÓ[\G)?ÙoDü‰Rú?×8
2ˆéH?øÜz9'Í@"ô7ŸÔq?ïå' Pˆ¿íAýa¿§Ë.€à©è¿ãÂÜôb=¿æä–bWŽ¿ïÿ´JõǘUNASNone?ï³á¹x?µ'—ó.éÖ?ƒ'³Šö-?µ'—ó.éÖ?ïãcñ6Ó?r̕æúÕ?lœäèMŒö?r̕æúÕ?ï†åí…)?…ÅQø(?ŽF"›F8?…ÅQø(?ï¿0zyÌR?b¿ÐŔÇ?€3á`Üÿj?b¿ÐŔÇ?ïèÍ"Kô?e;^oàÚ?g2ÝÃ*9Í?e;^oàÚ?gØ"ä?"žmôGZ?ˆR& ?"žmôGZ?ï-ŽÕ+§4?"ÆîEy?šN%Uc¯‰?"ÆîEy?ïT³1Vui?åZFÏE™?•i™Óy"é?åZFÏE™AGN4FGL J1416.7-5023¿ç|õÎ5@$mG8£µÀ9혮¸ÐÀ;øÂ!xÌ@ð·S=êœ@)†@÷A?À$œ—zÛh?Ӆ2ˆJ½@Ø.D¶é6?ø[‡`ﯿÒ8Àr×
¿Ú¬ìݎf
¿Ýê1!5.á¿æ
ÌÁå>¿î`ÊE3¿ïÿÿ&¦³UNASNone2FGL J1417.7-5028?عuŸ
ê?ÊßǕ¢¶?ã£E0zŠú?ÊßǕ¢¶?ڑ"ð&ª?ÊÍÊó±€?â·=±ì«?ÊÍÊó±€?ãB©Q·G?³ÑÍqö-?Ùzü­\'s?³ÑÍqö-?ç62ÀWڙ?§8Û[‡š?ѓšPJÏ?§8Û[‡š?±`1"a˜?°@5'f­$?íÝóùêð­?°@5'f­$?¥'«œM?°eÚ£›?åAo?°eÚ£›?¼ñ¸BëѺ?­OŽmøsG?ìaÈ÷¢…É?­OŽmøsG?ÂBñÞ{"?§²1¨à?ëoCˆ|!?§²1¨àMIXED4FGL J1417.7-6057?âñòSDÀ?ÆÊ#åbÿÀ9
>¼(À:G¨=¡K?@$x‰1l‰–?ý
¾4ƒ•K?Á…NÉf»Ì¿©ÂGBÒ/?÷€.>ì?ýîé':,¿‹?à<Û?îf^ê–¿î虱íM¿à³-ߌB¿äÊÜgtƒ`¿Ü'-ê
ËUNASNone?è­%ÊaZ?ͤ´ô®¶?ÍKhÖz—î?ͤ´ô®¶?ëñkŠ'•™?ÈÇÍèp?À:QÕµ©›?ÈÇÍèp?æ‹2Ñ}O?¶êI.y
~?Òéٚ]a?¶êI.y
~?íJ¤à/ç5?ªT"¡`P?µªØþÒÜ?ªT"¡`P?ç6êòv?ΜtcîÖ§?ѓÎ+Ð?ΜtcîÖ§?æ²0X¯»ç?ÔE7h]GÀ?қŸN ˆ1?ÔE7h]GÀ?èüß(ö?¹Ù°~7R?τƒ_à)?¹Ù°~7R?à‰úÀ%?Èëëd×3ó?ß×Öì
¶?Èëëd×3óAGN4FGL J1418.2-5400?ÏòLŸQ%@áÐÈ0À9ýH"Ô·À;}±CÝ¥@Š0NÒK@i"/?ÒzJHùn?܋AèÜy@èí¢/jQ?ø;O1¡¨?ÕÔ3~1´-¿ß{{áͺ޿è•.enâ¿ëOñå‹	´¿ïûÎ!á|1¿ðUNASNone?î‹Ãt«Åã?©Á«Á©?§CȶûoÇ?©Á«Á©?Ö:bÊÐ?ÌÉò‡¥?äÀbüNš˜?ÌÉò‡¥?ëçÛû'±?¤¤Ý9is°?À`õ9Â?¤¤Ý9is°?àß_ê~ìù?°g—¾`	?ÞA@+&?°g—¾`	?êŒc§M?Áê
Ƕ?ÇáÎsbÌ?Áê
Ƕ?¡N@PDi?±qÆ:÷?îëëí=I?±qÆ:÷?ÛêùYXòò?¸‡A¾À?â
ƒSS†‡?¸‡A¾À?ž]5TŽÓ?ˆÎítžH¼?ï
U¤C¹?ˆÎítžH¼MIXED4FGL J1418.7-6110?ãÿ[[àl¿±†SÁžˆÀ8!å±  œÀ9Fì\tu@ör~!Ãõ@¢¦¾EJ?àì){D?ÒXÉûa4Î@
% 8ð?øìWÿÆIP¿ïŒœ[ú?çÃEš>H¿è&@©-¿êcv'-"Ž¿í!­>¼ÿ$¿Ì‡´÷UNASNone?âLó@T?ÕRerËy'?ÛfWùç?ÕRerËy'?Ö&¹>òÑf?Ðr+¬ðÓ?äì£`†—M?Ðr+¬ðÓ?ÛïÇNÄÅS?¶¢&OíV?âXW?¶¢&OíV?ÕGÿó&?¼˜$A±XÜ?å\v€lù?¼˜$A±XÜ?áyÜ>YØ?×ţ͕?Ý
ÀGƒLP?×ţ͕?¡ß²¹˜k?°òÏ`'÷?îâԝs?°òÏ`'÷?Î|ÐÉd@$?µ
µ%·?è`Ëͦï÷?µ
µ%·?{Ä8h¤?{¼͓á?ïÈàwµªX?{¼͓áMIXED4FGL J1419.2-6029?ê´¼µ¨n?áöAÛl¢ÁÀ9"›vékiÀ:è‰ÁµB@!"|¨òýä@埱áŽü?سÑÞÚkq?'6¶ e©?ËÈWÈþµ?ü®¨Q˜N¿ïÒÒ4ëš?ïŸÄ UàÝ¿èçˆ9õÅ¿ä"ABÀnð¿å?¼xÁ²½¿íÜ¢ÞìâUNASNone?êˆÊ5æ
?ÍN9‹‰Wú?ǝÜ×(gË?ÍN9‹‰Wú?ï•-Ï1?ª¤"§¨X­?ZGÔgç?ª¤"§¨X­?äEó»_MT?·:ð`¸˜?×t‰AeY?·:ð`¸˜?ï2oÞ׉?ŒQ·Ër€?™¿òm@ì?ŒQ·Ër€?ç+êi•ÅÐ?Ͷœ\ ž?Ѩ+,Ôta?Ͷœ\ ž?ë{¾ìö?Ëpò¢Z™?ÂãéL&?Ëpò¢Z™?åÂDQØS­?½
(¤íh?Ô{w\OX¥?½
(¤íh?ç~Òè^'v?Âê%gŽ?ÑZ/BÛ?Âê%gŽAGN4FGL J1420.7-6701¿ìLÜ)a"ZÀ¡©É'†À:ùp™ÆÀ;™oJ:¶µ@=1¦ì@^]×M?ÍmíCdٞ?Μ
!Áñ§@a&Ö.?ùyÕú
¿ì@r`ð…º¿Â¶YÃÀ´'¿çtè?ƒ¿ç ÄÍ¿ëY^@'7|¿ïâ[>ê÷ZUNASNone?ï»Ó®úe?‡•5ÙÕ?HæÎ?‡•5ÙÕ?íÀ;mÙA?±Õe	Qî?±þ$'dø?±Õe	Qî?î¡ÙxE¥À?•9¯ÐÇì?¥âh~9X÷?•9¯ÐÇì?îOæ`'ÝÒ?Œ©þ¦¥t?«™÷Ò"ç?Œ©þ¦¥t?í€Z1¿?³&"8Õª.?·CÿÿT3‰?³&"8Õª.?áGèl*?҈Z¢7øÀ?Ýp/ß&ý¬?҈Z¢7øÀ?äÿ¹2*
‰?¸Ãq¹"¥ˆ?֍›«äí?¸Ãq¹"¥ˆ?ÞÕÇú¢jp?¾Æï	¯ù?à•®ÊÈ?¾Æï	¯ùMIXED4FGL J1420.9-6127c?烈^™úy¿Û T¾ôÀ9pAK#êÁÀ:oê–â/5@"Ž™¶Iþ@ð®Ý*?ÍÄn&NH?ªü8ö?è=Pù׳@{…UE¿ïÜ*7áï|¤ËüÃ5?ïø4SÅz¿æn'ûnj¿çnû€"dü¿Úÿr;†¾ÌUNASNone?ë]vÄ
9?ÆVeòùg?Š$ï׎?ÆVeòùg?ïµßþ$?•"0>|¶Œ?'º{֌Ó?•"0>|¶Œ?ç(vWº/?·\Ò'†°?ѯãP‹¢?·\Ò'†°?ï{74Zá´?†n¦á1±ô?™t£É|?†n¦á1±ô?íI‡u!6©?½íŸPùÓÒ?µ³ÄY6?½íŸPùÓÒ?î·¸†ÞH?´+¥ÓÂ=?¤"w›Þf?´+¥ÓÂ=?çñÕÒ§N°?»ö4z0Ó?ÐTZ±bŸ?»ö4z0Ó?ì¡i_ü%;?´ç·›Î'N?ºôµÖ&?´ç·›Î'N0AGN4FGL J1420.9-2431?ã¥"LðÁ@A¡ýiõÀ:^ÏO^%À<dëÄØí@çÒøŠì@ƞ<–‰D?ŁÂ7rˆ?È'øR¸@_Ô{í·?ùˆ¤~Ïê¿Ô²ŸÅ,Å[¿ág—ô}뾿ݓœº¶¿æ¸]¿xÑM¿äV›†Ù£¿ïô›]i¼UNASNone3FGL J1421.0-2431?ïÜÔ|n?m°«
Ê@?q•ÁÞµ?+?m°«
Ê@?ï$ïVˤë?Ÿ.!€©K?›b(C0¥?Ÿ.!€©K?謹…!Θ?€¥ÍlwB?…P­=†?€¥ÍlwB?ï@M;áÇ?rŒVKµ?WöZ;•?rŒVKµ?ï{¬%YÎ?ŒúMTÖÜ?Š{Yí¦?ŒúMTÖÜ?éÏvaþ?ÈK-"§†0?ÈÃóÂ&x?ÈK-"§†0?î%F6"ÚS?¢ûÅnð´Å?­«œœŒÐ?¢ûÅnð´Å?éx\wqô?°¬­Ê2{™?ÊŽ"9ˆ.?°¬­Ê2{™AGN4FGL J1421.4-1655?Û&ï]ps†@Dj}¿H€À;'œ%eWÀ<¶´•žbV@"á]¶"|#?×2¼ë®9?âΈ>''ü?î0öã Ì(@vA……@f&ż:¿·Ø\wûT¿ï ˆ¡#і?ìIØá®a¿ïúÕ>
|±?ïöÞï@5¿ç.ÄÑ¢UNASNone?ïù×qìV€?€Óv°ó"Ã?H¢9\"°?€Óv°ó"Ã?ïí5Uªßñ?tB… 8PF?bʪ'zç"?tB… 8PF?î¡öÇþÿ?™þ¸j/½?¥àžAÈB?™þ¸j/½?ïý\â"*?2§üP "n?5ìT܄S?2§üP "n?ïìþ\«–`?p¡å
ýkë?c£,Ž(?p¡å
ýkë?ï±úá)€?'ÄïDH?ƒG²)?'ÄïDH?îirx©›+?ŸBãéï©c?©hØrҘY?ŸBãéï©c?ïû2VG?Nò"É&DÐ?C6¦~õÚ?Nò"É&DÐAGN4FGL J1422.3-6059?í0Vi:£Œ¿¤Âþ*Æ[À8 6®è¶7À9­O©‹%@ FI²ül"@¢Ä?ò¥K´3xÓ?Ír‰Ië0@ƒðØï?þXËÁ	8?ï| ï
ê¿çú(»
,ª¿ã¼²F+]¿èëë†Ì7¿ìñ"b"4¿×r9Ù?¡ÖUNASNone?ÑCܯÿô?т›÷ÓòÂ?ç^'¨?т›÷ÓòÂ?à`=ƒF"?Ò0FÎ+Ù?ß?…ÒùrÙ?Ò0FÎ+Ù?ÛÙßü_j?¶F]ô þ?âwÐK?¶F]ô þ?âúbŠõÎ	?ÀøNg¹o?Ú:êcî?ÀøNg¹o?Ð 
óCë#?Ò77¯nÃ?çïù^
o?Ò77¯nÃ?³6ðK|â?À‡*­d…?í™!ö¹Ÿ?À‡*­d…?ÐäN¡×3a?´¹61´:×?çØ¯fP?´¹61´:×? yKÈN? ™º@w!F?îønë^÷÷? ™º@w!FMIXED4FGL J1424.8-6536¿Ê‹4"§ßzÀâ[úҙ•À:&.gòXÀ;€å¯º@´ºÃ{@ÀLÁy²t?Ù>Nî÷ð?é2užÎ_@p׈§@&{Ÿ^?º,×#'×?ïè¹\­€¿ëÔ.béÚ¿çÏÚ¾|ýؿؓ²Ï˄οåÛíÎmUNASNone?ï"îò32?©jÅG|©9?›¢!·ç‹¶?©jÅG|©9?쮺:x÷¹?ºèä+Ik?ºŠ.,8B<?ºèä+Ik?ìGûÑ8?¥Õ©
#?½Çp'Áv>?¥Õ©
#?ìRû‹.ÐV?¦¬ÚËà`?½h#¦‰}S?¦¬ÚËà`?ë>ù§˜­-?È)B
ì|À?ÃaKL?È)B
ì|À?ܸhåzKS?Ô#9Epøf?á£ËBÚV?Ô#9Epøf?åöÈ{PП?µÃ­‰?Ôo	^^Á?µÃ­‰?Î|ÙûŸa?ÁzÙÅ® g?è`Ɂ=Ø(?ÁzÙÅ® gMIXED4FGL J1424.8-8012?ärÎa!ƒÀ2Q֌i/À;¤š~›çÀ=IÄòø6@Fé—îâ?ÿé={‹'™?ÕªÜ3?ïÿ踻Ð@m$
<ÿ?ý^g×®6¿ç{½ ´ëÛ¿êá|¢¿·†ƒ'F>(¿Ù‰ÿöÅÅ¿ïþ¢½"°S¿íQ&ΠâcUNASNone?â2tàÛ?Ð#Šõ£?ۛû>äJ?Ð#Šõ£?å·½x"\
?Ê]‹}Ä?Ԑ…ÙGì?Ê]‹}Ä?äÚÓÇ׉X?´&û†¥td?ÖJXpPíP?´&û†¥td?ãwõÉEY?´SZڒ?ÙþmuN?´SZڒ?Û×+ƒog?ÒݔK¸ ?âj>HvM?ÒݔK¸ ?Í¡Ê*0*??Ës<Ð7\Û?藍usõp?Ës<Ð7\Û?ØQëÀT™?¹•v°×Ù?ã×
@Õ³?¹•v°×Ù?¿e30g?®R = ?ìY™ó ?®R = MIXED4FGL J1427.8-6051?ïBò\ÿÂæNh˜Å´À7™ʬaÀ9æ?Pwç˜@,ÚÏÄÎÒ@ùü£T-?´õæ °Ï–?ÅÅxDµ;·@9	ۂr?øÅqœ+?À)nä9P?×´ÿüz¿çÚcŽDÑÁ¿êÊ*ü-©¿åŠØ5¶›2¿à¨<_+߂UNASNone2FGL J1427.6-6048c?çzZH9Äa?ÐÞüB±£?ÑKoŒw??ÐÞüB±£?ÊíRH¢0A?ÂQ"ÈãDo?éD«m×sð?ÂQ"ÈãDo?àdÛؔ'Z?·‹U|;îK?ß6HNÖÛL?·‹U|;îK?ÊÐuó;d?­ÔìoÄ!ò?éKâƒ1<'?­ÔìoÄ!ò?Øz/Qã]Ä?ÐxÊcˆ\þ?ãÂèWQ?ÐxÊcˆ\þ?ãy6¢©c?—ªC‰võ?ïxä62…?—ªC‰võ?Þ©"°‡?·…T~£`?à«6t'¼?·…T~£`?sù(qJ‡n?if•Ydz:?ïØ
¯Yä?if•Ydz:MIXED4FGL J1429.8-0739?…bþȊ'V@Gìd^NiðÀ;fBÀ<ýÔ£Zã@X6hqÙa@UinX£/?Ô'Ӄ 3?ì|p(‡Ç@[bâMg'@Á*WA…[?íħÈ0†?ïó'?	*K¿Û&ÕøÎ]¿ä՛=ÈK¿íö9ãPœÑ¿ïÁPb#UNASNone?ãç»­ˆ?ÆZýÀ?Ø0ˆ¥øÄð?ÆZýÀ?ãùHƒŽ?ÊTY©>¨1?Ø
ãánøå?ÊTY©>¨1?éM±·{4‡?°ÀòWñ—?ÊÉ9"-ã?°ÀòWñ—?áÜWµ&E˜?³ÅÅU5ñ¼?ÜGP•³tÑ?³ÅÅU5ñ¼?д¬ë?Ç—œz}?祩Š}qñ?Ç—œz}?Ê_}Oc?É Íaêx?éh>à»l'?É Íaêx?зÜAð÷?Àeyv¹oÎ?ç¤7'ß"?Àeyv¹oÎ?ÀÐÀd'?ª"ÁBÆrA?ëËÏæÿö<?ª"ÁBÆrAMIXED4FGL J1431.0-4432?êüjÊhˆ@-Ê¯¼ÎÀ:Zy¯ïFtÀ<"¢"=_@ˆ´™û@À#Uož?Òø®6Ý?ÄïäêOêy?òåQÉ oâ@ÉÎÖ俾šP£±uƒ¿éÔÎX¾7¿ä+¢zé«*¿×")ÛE¶n¿ëQ(¡´Æ¿ïñwÁØ}UNASNone3FGL J1430.8-4434?ïõð竗À?Pìmƒ½U?T0-?Pìmƒ½U?ïäüRò?xoÈ	ݏ?kåt.ž?xoÈ	ݏ?ïÇÞÁ@ýv?zõÅ>Ž?|Ÿ}
è»?zõÅ>Ž?ï÷*Ú@ ?6_üÖusŠ?Pý©èŠ>?6_üÖusŠ?ïõˆ{AÈU?SZKK6?Tï	'9‰?SZKK6?ïP"ë4?£‹Íçʗ"?•íb™}??£‹Íçʗ"?ï|傿ý?¤™‡8©?cO¦HŽ?¤™‡8©?ïßõƒ¥;Ž?\³=ôF'F?p>Hß´?\³=ôF'FAGN4FGL J1431.5-6627?¾h"x~}À	‡Æ2~ØÀ:CÇE¤NÿÀ;±•ìeïH@äjÔ4J5@—dj㣩?Ï_T¹À«?Ì!^IŒf@BÌÛæED?öAkBS^?í:1…ý¿à¾Ý®‡¿èDƒBL"¿å"M!pèö¿ïÿò> w?å6YX`êUNASNone?ï¹Ä"jtN?~bú÷©£?Ž÷\ú|?~bú÷©£?ízÏAFF`?¸nïœÝ%?´)…ôþÿ?¸nïœÝ%?îí(‹J²'?'	 ¾Ï?¡-wNÄrÜ?'	 ¾Ï?îq:S–‰?ŽŒi(Jž?¨ï<_p?ŽŒi(Jž?ïæ{/ÝO?›#ñ5‡­P?ã0"Üì6?›#ñ5‡­P?Øñ#óéá?ÑǶ•í?ã‡xî?ÑǶ•í?è1F†Í;?´›Áœe?Ï:åäËÇ?´›Áœe?àg@ ?»Óž£ÉP?ß1ïãõÁ?»Óž£ÉPMIXED4FGL J1433.8-6357?îÉÐ"}6À
R˜˜—;À:áÍ:°ÕöÀ<§³Ó׃	@GpxŽ@¸îÿ&¼,?Ö×.Û4ă?ïÿ—?LF*@
φþŒby@6Ö)—Óò?îª÷?g?ïä;û…G?°1æA'òa¿çx!m
¿íñ܆~3ã¿ïÿ\‹/ôUNASNone?å#&Š<æ?Ê_z[]@?Õ¹²ëdž3?Ê_z[]@?䛝ÞUi?͵¿Y>,?×ÐÈÄCU.?͵¿Y>,?ê¯:Ìjã_?ª°c_ Ïn?ÅCÎTr"?ª°c_ Ïn?Ø¥oEˆt?¸è¸k/¾?ã­H];ðF?¸è¸k/¾?Ïx 
•ö?Æ=DÇò"?è!÷ýZ¼Ã?Æ=DÇò"?Èä?ãÆÂ?ɳҕc©ô?éÆð<ÇP?ɳҕc©ô?Õb§Î?Á=ë'æF?åyÎÿñ¬?Á=ë'æF?ºù-ñÞ\Ë?«4Ðõ®ö×?ì ÚAÄ4g?«4Ðõ®ö×MIXED4FGL J1436.4+3900?àèV$¤Ð@PG͉‹.À;¥á¨&$WÀ<ë]à…ç5@ `¾$ƒæ?ÿÓ¯tÍ1w?ÎÆCÜ"Ö?¡SÀúå?Ӟ¤Zè®Ö@3Ý	°Øпëkô0õk?ä(½ž†"X¿Ü³T€µÇø¿å†žEÑ¿Õ½ÄܓiT¿Ó±<MŽ(LUNASNone?ïý{9mp,?,
G'Õ­?4&2¼ÍÛ7?,
G'Õ­?ïôÑòâ¿?["Áacç?V]Ãù>BÏ?["Áacç?ï鮬4Y?bo…â–,d?fQSí+~Á?bo…â–,d?ïóɞ͓¥?BBE¾µÙ?XlÁî¦'#?BBE¾µÙ?ïûÕç†?'?<Ñûìe:?@¨a—Ù/£?<Ñûìe:?ïÑÄ8²+¿?€—±¾?w㏌Èv?€—±¾?ïâÄ$©úÝ?sŸ&­$î?m;Û3©
?sŸ&­$î?ï¿m\é~Î?rv¸æµZ?€$¨Ë¬x?rv¸æµZAGN4FGL J1438.0+0219?ÀJó@;ã@K6-œñ<ïÀ;MÆF ÎAÀ<¦MÝÙe@4œ´V3h@Y¨Íê>?Ñö«XþÒ?ŊnÙQ•t?ïXBKÔê¨@¤–^PÃ<¿íN¶È¥ ?ï÷䨋¤ä¿ç‡âg^3¿áv"@Áç¿ä©Y?·P¿ïڅAÈÍ9UNASNone?ïþã>"ª?†¿¤D_?!Ìœz—?†¿¤D_?ïñ8
ý3?bÆ:yßþ?]ŏúÍ?bÆ:yßþ?ï禀:€?db˜©ï"?hY'Ec=?db˜©ï"?ïúëªÍ7p?/bøÿzø?DQT|"Ë"?/bøÿzø?ïÿ*\l^ð?{ûAo"¨?´y¢" B?{ûAo"¨?﹗VPø?L"Æ/«"?š*eꢙ?L"Æ/«"?ïÊØڈ]m?~;x]~?z"'¬³k?~;x]~?ïçä¨$'?^Wª~y?hìe™ßP?^Wª~yAGN4FGL J1439.2-5142?ߤú©\Ó@ºø>jžÚÀ:"…fîÀ;¬ÿðÇô@ìüÝ5М@®}Vlô?ÐsÀA#6?È
‰Æ½¿?úRš×‡;?ýàwÇaÓÛ?¡g"@
ƒ™¿ç<ž_æð¿ã«4–àµ¿è«e©¨–¿ïÿúVrÓ\?Ó_o|9·\UNASNone?Í%-?ŒÂ0¾C/?‰Y½{ì£?ŒÂ0¾C/?ï'˜ƒL®¸?£ÆiJ5G#?›ï˜!÷?£ÆiJ5G#?9eÈ?•k«ÈæÑ??¤W¼pÝXx?•k«ÈæÑ??ïr)a4?w"ä>ˆ›?'¿¿ûCˆ?w"ä>ˆ›?퉙Éaª·?¯p‰‡>¯?³³1¶<"Ä?¯p‰‡>¯?çv5E©yÙ?Ì¿²V˜¬Î?Ñ•t­N?Ì¿²V˜¬Î?çóìÐQ?¶©þ\1?Ðö'Ü_^?¶©þ\1?êBLÍ|äÇ?±wÃÂX?ÆöÌÊlå?±wÃÂXAGN4FGL J1441.4-1934¿ê" ½""@B¦µ(À:ñ"Nü½À<{Ó"Qc @!-"Pª<?õdãåFn?Õ3_¿-R?à
¨š¾\È@"•ƒŠcœ?ôùkjÏ?½|­_I<¿ç9äàõ?ؕAED­¯?°O\8û¿ÇRl´^@þ¿ïýʀÂ2?UNASNone?ï‡C(l¨?²‡ñA­<?Ž/9yTqö?²‡ñA­<?íLëÄ<c?¼®Mg´;©?µ˜¡ÝA?¼®Mg´;©?ïÒAßQ?"6þÍX–x?žå·Ç…yÍ?"6þÍX–x?î½õ³ƒG?
áºÑ"á?¤ ®×[€‹?
áºÑ"á?ﮈºµYO?†?£Y	?"]ÑKÊtQ?†?£Y	?äIθŠJœ?Óp‹7_?×lbŽëjÈ?Óp‹7_?îxŒÜFèG?Ÿ.Û%NDç?¨w2<mb'?Ÿ.Û%NDç?êAò,œ"õ?·l'-Ûõ#?Æø7Mì+?·l'-Ûõ#AGN4FGL J1442.0+0732?Ñ0vY<v@L£ä`gHäÀ:݃¡àøÀ<o?v7"Â@2G?ڋ|@aÓÅ'j?Ð1¾"ùò?ÕGfÿ1?ÿ0	}WC´?ûQ0αÿ?ï¦ÿ]ꏿã°É–·g
¿á™î=µÃ¿ã–€À.Ù²¿ê_`—Ì:¿ïƽ FUNASNone?ï"
çS{?•âHƒ(H[?ŽøýIš½V?•âHƒ(H[?íêú1?¶þˆ¨C?°¯»Sx?¶þˆ¨C?íí8P0N?¤ǔ{8?°–=X?¤ǔ{8?ë7µ'§8?¢"8ì´?Ã!)÷±c ?¢"8ì´?îÆiË0ý?¦£fK3f&?£žÙa•":?¦£fK3f&?ã*˜ý3ê?ÒÕz]
¿n?ÙóªÎ˜,?ÒÕz]
¿n?ë‹Oìsӄ?©‡æçö·?ÁÒÀN0±ñ?©‡æçö·?ۅ=zX?·k¦Þm?â=ar¿BÔ?·k¦ÞmMIXED4FGL J1442.1-2800¿âs'ó@<ÌRş±âÀ:|غ@ÙÀ<A˜ý'gv@éN
'@cq|D=?Ƒf"ÄJr?×âûã:Í[@¶ˆ7q†U?öKÐc\0?ß¡—_,¶A¿Ýœ"`IÁÀ¿æ¤ªÚ3½¿î»CÝOÒ¿ïù~¿\¢¿îvª¡~ÀOUNASNone?îÞÿ…ÂÞH?° 7™'?¢ bŠ?° 7™'?ã2ðùãía?Ë«Ê@!û?ٚ8%>?Ë«Ê@!û?ìþ·*¨?¡p ±MÛÏ?¸
F¯˜²µ?¡p ±MÛÏ?歙p©á:?­2GÔ>«î?Ҥͬ=‹?­2GÔ>«î?꘨i&p?Åm|¿2O?lj^[f>?Åm|¿2O?Á1á?Ϋ?ÄÎée<x_?볇¿°U?ÄÎée<x_?ã¤òÔ&?»jy¨Yó3?ضW³ßÛ?»jy¨Yó3?½,S/§ã^?¥ºÿƒ?ìZuš"?¥ºÿƒMIXED4FGL J1442.1-3707?ìxþS­|%@4­3;–¯À:ÏeóSIÀ<"­Ù©T@ 6šn*Õí?þ'Xœ‰8?ȁ'ºýíV?ÁmhxºPô?ù¿ë¨Z&½@\"H?ïëy@×æ¿âúò¿Ðû¿à¥lZþ¿×i#°q¿à™RÓº}¿æ±·û"pUNASNone?ïý*T?,g.Êc·?7V±_ÁÍ?,g.Êc·?ïÒK$Ò®t?~D…MÙ¾?vÚm­V1´?~D…MÙ¾?ïéãÂ?s1==±'?fôÙ¿Î[?s1==±'?ïÛm©Ñ ?Q"í²Õe²?rI+/òa?Q"í²Õe²?ïö­òI¼•?K‹ˆɾµ?R¤QÆ<?K‹ˆɾµ?ïŒH´`?§Pç-‰?œ.vðS8?§Pç-‰?ïæç4y{¹?sؤɱæ?iËVi¾í?sؤɱæ?ïIbhÄ©W?€ôÇÂÁ?–Ó²é"£+?€ôÇÂÁAGN4FGL J1443.7-7037¿àUÓ):êjÀ#‡ãÑÌÀ:
j»_¼ÿÀ<¸{0œ@rôf¹@ó¢#«×?ÁDyA_ò?À?PøÀñw?ýò–³5L@ÙÌ¥	º>?ïáö?6÷Ž¿âÅõåÊË¿ä_²?¿à²üÁ‡¿è½/Á
ÑпïÿüoQÇsUNASNone3FGL J1444.0-7033?ïìgB•?v8Ó{%±ß?c˜½L6oj?v8Ó{%±ß?ïß÷ëo¶W?yá*™[@?p
WC-?yá*™[@?ïØ+Üìnm?x}tTý'?sê"g±®?x}tTý'?ïÂ	>1?_ì¿6±Ié?~õ{".{€?_ì¿6±Ié?ï	Jƒu?Ÿê7,AE}?žÝö²ý­e?Ÿê7,AE}?ï~®Èę;?ž""­¥õZ?*&åµ
•?ž""­¥õZ?î™[!Ü? 9£Ì¹±±?¦n:Ošª? 9£Ì¹±±?î®t
z§?‰ºx˜_`L?¥¿X^Ւ?‰ºx˜_`LAGN4FGL J1444.1+7601?È» ày—@C˜P%"õÀ;›Ãèø|~À<÷Â,_Ú@QRÖç'Ü@E]Ø"k?ÔZ^ï®?ËC扷N`?ï>~jê?þÅúˍ³¿î¨f»ö»´?ïüKuIX9¿ÔD­®úSï¿äÏBrì1¿ã1ÿ÷œ"0¿ïý³¥ÝuUNASNone?ïôÈ«nÇù?Oáül{öÈ?Vn©5­Þ¸?Oáül{öÈ?ïåܝq·Ë?r"ÍáP¹?j#bI¶?r"ÍáP¹?ï¼­¦•Ë?v£!OÅN?€Ô–xZH?v£!OÅN?ï¹fUjÒ?cÚÇ£óœ?¦~jMU?cÚÇ£óœ?ïðڞ¥$Æ?Y·þ"×(j?^JÃ-?Y·þ"×(j?ï›6°@O?•a±åË£?‰=ò^>À(?•a±åË£?ï&|؇"Þ?'‡£êõ?›0dæx^O?'‡£êõ?î¼[Î1ü§?Ö3™X®?¤:Cp™?Ö3™X®AGN4FGL J1444.8+3645?ä‹;¿…@P
·AJM+À;	5œ™ÿÀ<r@žUÀý@xi^hk#?üŠÉ‡î"?ä!j³Ó?è)¬¡´N@8³¥´Z@͓´RW'?ïh<>õ‰/¿éHQ¨i@5¿á¼ˆ¿îm¿íQ‡aˆ±¿ïí•Ïà}"¿ïøtP3ôúUNASNone?ïÜG¢'!ç?•À³þŽ¤?qÜ.¡¡x}?•À³þŽ¤?îk»lý¸?²bËg¢©?©DFöœo†?²bËg¢©?îJšG`ß
?•ðþw˜&£?«V[‡^Z^?•ðþw˜&£?ë8¶0d]?§|órqð?Ã'>n‹à?§|órqð?ï_j§ó?£¢'S–{?Ÿ"À"Ï¡?£¢'S–{?è,®
?Í!;ø1]#?Í¿O§™GË?Í!;ø1]#?ì"+A]~œ?¥ÑæüÙ?»^¥õ?¥ÑæüÙ?áóômòï?À,`tù–?Ü$!Ð?À,`tù–AGN4FGL J1444.9-5939¿ìTۓRò?½Hô‹(À7à°.0"óÀ9Õ~;oA×@ס–¾@»œ=¸È3?»ZÀ?ö?×)±>y@ Vlô!?÷ɋúŸ™?î]/Ÿ¾w¿ÎIÊäÀ3Œ¿æä:og—¿ë^u×±ç¿ïÏk¾Td¿ï÷ú"‡UNASNone?»¯ö6#?ɍŸ.Ãs?ìŠ=9=Ü?ɍŸ.Ãs?³6¾[gQ?­&mŸb'à?í™>4"?­&mŸb'à?È?¾ëbº?²ê¯±•0?éð=ÐE'Q?²ê¯±•0?}u¾b™¯Á?kÙpÒ®–´?ïŃ^ˆ?kÙpÒ®–´?žß#tJëç?Ã&•K?ï	äB+Á?Ã&•K?'º'f
^?"Ó1T†¡?﷉ŠMC?"Ó1T†¡?®3¼Ö@±$?£'©Þ{Äô?îÄ2Ž6~?£'©Þ{Äô?BÄuW>ü;ã	K?ïÿ²ôù*">ü;ã	KPSR4FGL J1447.4-5757¿ëj(1™Íh?ø^Ç»ëÓùÀ8‡¾[ðÁŸÀ:¼ÏJ«@j33fà@ký."h?·R‹íš<?ÜVômû†@û*ÂKi‹?ú"ŠÑ¹õ?ïõÄ"`¿ÓÏ© Z8¿æMOÿqº­¿ìzÆ:"‰¿ì¨õŒßvó¿ïþp]áÁUNASNone3FGL J1447.3-5800?ˆàxBŠRÐ?šQ|Òìÿü?ïœ~•%?šQ|Òìÿü?³|´ðšÙÌ?­OW.¤¨ø?íiaÃiw?­OW.¤¨ø?Ä €—Ù¿¾?°òR¢¢?ê×ßÚ	?°òR¢¢?žetà
¬?ˆ­v+'?ïÔXÿ—ó?ˆ­v+'?,—}î??·>˜—?ï‹Oõ"I×?·>˜—?¿6!Ý?"Æ'ì¬?ï¹'í¿?"Æ'ì¬?®"aLDRö?£Õtבx˜?îÉë?£Õtבx˜?4"eº×ÈM?*G#c=ÿ?ïý{³L£?*G#c=ÿPSR4FGL J1449.8-5923c¿ï[U æ?·a» ™VíÀ8¨f±åÀºÀ:B†Î»ºV@¥{Ð'@jTà,%"?Á¾x÷¼Q?×Xö;[á@•!4y@¦ã™—ì¿Ý'ހÔPп£TcÀªæ¯¿ÜßLÁ¤¥'¿éFÝÕ2ÌÜ¿íÏr™{¿ïþ€£ÿN)UNASNone?ѵš<gö?т`ÿ"Ÿ?çt%2áÌ?т`ÿ"Ÿ?Ôg4©³?È\Ç^×Yv?å÷Lxå«&?È\Ç^×Yv?ОJ3Ë?±]ˆyHh?ç°ôÚæs›?±]ˆyHh?ã#TîÄÄ@?´ƒ_£,)$?Ù¹V"vw?´ƒ_£,)$?",Å}Dœ?°¼ !Ž"/?ïgvšÎ?°¼ !Ž"/?˜=,¥2P¡?¢üe•ÖÍt?ï>šºð›?¢üe•ÖÍt?¢±ªœ5-?—̃züÔ?îÔåVuFm?—̃züÔ?¤~ÎÍd©?"wüNj?î¸U?"wüNj$MIXED4FGL J1450.8-1424¿ã3Ô7œ›Ï@C®Ûʖ'À:ñ9>/HÀ<«©Ìíƒü@¦o;÷ýÓ?ÿ	‡ƒ U?ËzÆ[¯S?àšIÂÁ±@b.ä¬?ýZæØñ~?ïÿ•!îZ¿ß°nh@†¿Ðä¶Î]Ç¿àd"‰—Ã׿ïÿþó…õ¿í<¢¤@UNASNone?ëk×óé¿?ì\õyiM?ÂR 0Y?ì\õyiM?æ×ØÀ?ƼŠ—?™•?ÒQÒOîÐ?ƼŠ—?™•?èÐõT†ô?¯Ñ¸—Q9?̼)ú­ä2?¯Ñ¸—Q9?è;•Ôæ¹?§CHíï,)?Ϩ­øe?§CHíï,)?ç×üÖ!V´?É"[#$?ÐPS½R˜?É"[#$?Ï×Ú°BÛû?˼õ³i¾?è
	SïI?˼õ³i¾?Ò"ë9?ºkª@ìë?æú=ÿü
c?ºkª@ìë?ыŠ?è
?°Ë'W°+‡?ç::àÿú?°Ë'W°+‡MIXED4FGL J1451.6-3726?ÙäԊAþ@3‰ ÝDÀ:†\ø(›*À<*ÐíýZ@Ÿ¹"uö§@ž¢ûB+?ΏbÞòi?Ø}VÂÚZª@'!ý€É¿@~AÉùÞ©?î¼´áɉ ?ëmô?,­¿ÚLǤùv¿è<¦ÿ³©æ¿á+þöë"H¿ðUNASNone?ï±V½YšÚ?'òõ\¹@Š?ƒªPºo_"?'òõ\¹@Š?íëIc›·?±1zS0¾4?°¥´ç].Ë?±1zS0¾4?îœ
C(¹?–[!{à'?¦?[Ëñr?–[!{à'?î7 n4é?¤9@ú'N?¬ù$ãk?¤9@ú'N?Ž–[L?¤ü	*•¿?¦"'–I?¤ü	*•¿?åÊ;éÌH)?Ïv¥ðj?Ôkˆ,go®?Ïv¥ðj?ìm_÷-ì?©Éã–//?¿ü•F¢?©Éã–//?ä­Ì[‡?ºJdR:	'?Ö¥ÊgËHò?ºJdR:	'AGN4FGL J1452.0-4148?㳘àOû/@/J^±¬À;$üȼÀ<ƒ|Æúû´@ Êì=ÖOX?ÿ´W£U?Çú–È¿\…;T%Ï?™ÿÑån@T$Ñp |?¾=‰ÎJ{N¿áû¶úÓpU¿Ú׶_Íðä¿ÜsÿÁ–¸¿¿Ý<ñ¢ðŠ¿ðUNASNone?ïû=Ø›½?8{`NŸY?CžçYá®?8{`NŸY?ïä^qOxŽ?w •%‡t?k¡ŽqN¢'?w •%‡t?ïì0W-0?b…É&¨Ìð?côϲq¸?b…É&¨Ìð?ïø5,?4øí"ÂX?O·ë¶ì>™?4øí"ÂX?ïûÈÿžíR?:ŠòiøŸŸ?@Ü|È^?:ŠòiøŸŸ?ïi|N–LC? Í¦õúLö?'Ðv)Æۙ? Í¦õúLö?ïèü]fÁ?rf˦³
Ù?gbÍ4f½?rf˦³
Ù?ïޘà´Ð?`l4ސbô?p³ïôؤ-?`l4ސbôAGN4FGL J1454.3-5551?å½Åo$>è@äI:ÜtàÀ9ö¢ñ10$À;Xù"«ô@"£ÊŸöÖ@zh˜q?ф}*[?Þ|´†"éß@Œûü@_œ"JÐ3?î…ëÃ¹ÿ?°Ý§Û¦¯¿êóæasbx¿éÙ—â¿ë
´Û¿¿ïýf],+UNASNone?îØÀÈ "t?¦»e¯ýÌ.?¢sóy¬5Ë?¦»e¯ýÌ.?遆¹~M?†¡§?ˉùåÎ?†¡§?ìš]ÁÒî?£ôAo†×'?»-ño'?£ôAo†×'?ì_A­ÁÞ?œî•³?½ó''ñ?œî•³?å rß=Š?ÈÑúrS?Ô¿àA"ì?ÈÑúrS?Å6¯ù=ª?Æ®êÑ?ê²~Ô°•?Æ®êÑ?á?ÿ5Z?ºÞö–°í.?݀•ßÙM?ºÞö–°í.?Ñ[/¢Qq?µ[—Ñ#×?çRh.×H?µ[—Ñ#×MIXED4FGL J1454.3-3946?ìX½ß
@1<¯bk/À:ϳô¬æÀ<̙¡&@ýˆf# @ÿMzÝð?Ûô°@¥¾?ß?p\‰?ø)&i÷@´^»!S¸?ä»!©ô¿éî4Ïëe¿ãç ÏÃÍ¿ïÿÿ>¹ú?ïÿ‰ñÇ®?ã–!‰"UNASNone?ïì¸æøl?¢	˜vñÞ?cG<7£æ?¢	˜vñÞ?ïÕÊ9"?ƒ‰›yâ|ß?uãdu–Ì?ƒ‰›yâ|ß?îTØ3«©?›.ªëÚØ?ª²|ĕ©r?›.ªëÚØ?ïÿ¥Ó?
Š –—?f¼ˆ±?
Š –—?ïã+¬(?z	g
â©?lpÔ1"ÀR?z	g
â©?îBq¢Ëg?·)ú±ÁÁq?«ØåÜS­›?·)ú±ÁÁq?ë<"VÛÈ­?°î‹ÊŠ8?Ãv¤ÝL?°î‹ÊŠ8?ïÖ>Éûrc?{ð•!ºbÛ?tàšìù:°?{ð•!ºbÛAGN4FGL J1456.3-5419?ﮜcVE@ي¨exÀ:Symª'†À;Ôj:0}v@Ið<h'@ž˜ÜÛ7Ê?ËOž"ë<?Ú6=©¯@}¦Z?þ)Þb÷F?êQMÀR@¿çœ'0>Œ-¿á>ƒö¿æ¡o† ˜'¿í«a·€	¿ïý\á0UNASNone?ë\åJRµ?·ÎQ$Öf8?ŒkþÖµ.?·ÎQ$Öf8?âZFï—kÜ?É»·¤z%é?ÛKr Ñ(I?É»·¤z%é?ëyç…	ê?§ÞkzŠPJ?ÂaëØUÂ?§ÞkzŠPJ?èF©ÁÍ?¦Q‹]Í­Ì?Îå[ï"øË?¦Q‹]Í­Ì?݃Þ
P«?ņÂÃÕØ?áq¾ú׫?ņÂÃÕØ?°"v×?¶|ç3wÉ?íþ
³•Õ?¶|ç3wÉ?Ü2]IKe?»øÄwhÂ?áæÑ[ZwM?»øÄwhÂ?Á¾ª¦˜kØ?¥8Õ ²?ëUVYå
?¥8Õ ²MIXED4FGL J1456.4-7129?dú» :)ÀÀ&`®–À:ðª¦1W'À<m¡â=wZ@m®˜YR­?ÿ¶JêßÝ?Òk–|ÚÑ?ØEAþ}@pë?~›@uVSsÅu¿ïýРkð¿?ïÿ¶~¬®I¿âå{ð;g¿Ùó:à%Å¿êmbnŠ!W¿ïþÇ1¾UNASNone?ïÆ%âov?|]vÓóéæ?|íúWi/?|]vÓóéæ?ï §²Xy¶?Œ	¬û@ì?‡ÖcZƒ?Œ	¬û@ì?ïq`)º?üâV[]G?ž1Ôñα?üâV[]G?ïc˜ºîË?t×ZIîz¸?"Lì'?t×ZIîz¸?ïkɹ`Î?Žª?1­ÇÛ?'†ÈξÔ?Žª?1­ÇÛ?îEš~úd"?·yQÕÖN?«¦X5Ì?·yQÕÖN?í/"äE?¤§u3åˆü?¶ƒØß	"Y?¤§u3åˆü?ì#eéF‰?¨ëñKÏdÁ?¿Îäе˻?¨ëñKÏdÁAGN4FGL J1456.7-6050c¿îrH1ûƒL¿ùqÕëYÎÀ;e߅65FÀ<1vßZn@&£¨žð?ó­Â*²[1?Ê+?Éą¿¾Þ㥬Lz?öy^«‡ç@Êò4:o=¿ïÖHaÇó?ïí,•<=¿ì÷³•Ä"¿êzàñÇÙ?·4£ ®Œ¿Û­ë=ÑUNASNone3FGL J1456.7-6046?ïþ†ÅE]Ç?A	\HÍó—?'"¬'{¶r?A	\HÍó—?ïµk2d<|? ¶Š5
"R?'¥3wÆöø? ¶Š5
"R?ï¾e50ZÞ?~Û8Ø\­?€f²ªJ`ˆ?~Û8Ø\­?ïö8ÄÅ¿?TÉцIÍ?SŽwÚ³'|?TÉцIÍ?ïúËL¼hž?J-35RÅd?DÒÌ»æè°?J-35RÅd?î'	ïåM?¸*ˆ‡iŽ?§ßa‡t?¸*ˆ‡iŽ?ïc¤¢CY?–`•q4Ù?"‹'–Ìß?–`•q4Ù?ïŠjÅѽ?•0"bòd?eN¼»,?•0"bòd AGN4FGL J1458.8-2120?è°+†QÏ@@H‰ÁµA–À:eJýTTÀ<Ê8Ö?@ªqùílU?üäœ,ý?Ä·.jv–_?Ûë<äâÃ.@à8ýw"@p^ùÞ?ú¢É¿eQÃÂ)"¿É|ƺš¿ãÕô~A¤e¿ë6zæP+'¿ëü?¶Ï4†UNASNone3FGL J1458.7-2120?ޟìùÐi?Éú6[ß>?à°	ƒ?Ì?Éú6[ß>?寨öý?ȳEð­°0?Ô ¯ÂÐ?ȳEð­°0?ß6ÀË%œŒ?´æ¦D?àdŸšm1º?´æ¦D?é'â?¤ÂtD£Þ?Ëb—Üw‡?¤ÂtD£Þ?º fŽ³ã?ÃGV…±Ô?ì«ó.>	"?ÃGV…±Ô?Ìú:V› ¸?É£cœÝpß?èÁqjYÒ?É£cœÝpß?±½p¥ŽØ;?¢
QüeÛk?íÈQë…¸?¢
QüeÛk?Ôîãû	£?±ÿtWg[^?刎{t.?±ÿtWg[^MIXED4FGL J1500.1-5846?´ Á÷T?¶j#¤
ÖÀ8®n‰J—À:'¤ÑÜF@¶ßªõâp@7րªµK?ËØF=&&/?ÈL«êªr?þ¦îœ*m'@%ýžü¯é¿ë¶D•[Fx?ì_>Sù¿è2í"ñÚ¿é¹Õ䣃'¿ê1y¿ß~€¿á´¬¯öÓ1UNASNone?æF€ºG?Ñuö'Â)?Óûrþ‹qõ?Ñuö'Â)?í×ÎO¦'ê?¶hÌ!4ó?±Aƒ<´1?¶hÌ!4ó?à܆cÜÉ?ºâï+¤ý?ÞGÌó8Fm?ºâï+¤ý?í¾€¥›ŸG?žÖ‰ï‹?²úÓ#Ç?žÖ‰ï‹?àמQ[´©?ÎKR"ÄÀ?ÞPÃ]H–®?ÎKR"ÄÀ?åíd TÍü?Óyz¿'·n?Ô%7¿Vd?Óyz¿'·n?؞ÃuÇ=¨?½lÿÜ.?㰞Ea,?½lÿÜ.?Ù&ˆµ›­Æ?Ä ·:i]g?ãl»¥2)?Ä ·:i]g	MIXED4FGL J1500.2+2640¿ÍºŒ';@N®"î9.À:ìðó®À=á{°z‡@ï¿ÿ^ðP@^@ÈG,?̈ѠF1?ïÿöàœj@Ú­æW¸N?þ äßh/ê?ïàÇ ½û#?ÖLòãÕ¨¿äáƒÞFqÔ¿îö'"׿ïö4osUb?ÃVú£ӀUNASNone?¹ˆªç}[?Èf"%éJ?ëQÕF ©?Èf"%éJ?ØF
oÂÜ?Ð?†cí÷P?ãÜùrÈ'?Ð?†cí÷P?ßn"³?²º¨©t0"?àHôôð=¦?²º¨©t0"?¤è•"ž°?Ž¾JÒ+ô_?î±~vÂBõ?Ž¾JÒ+ô_?Ñûlsé
?њÚÀðŠ?çIÆ?{?њÚÀðŠ?¾Hõð»?Ä#ôkH?ì=¶áAèœ?Ä#ôkH?Ôþeø±ð?³(^‡¹Œ?å€Íö§?³(^‡¹Œ?U7h?Jºæ‹ÝÀ?ïõ7äa­´?Jºæ‹ÝÀPSR4FGL J1501.0-6310e¿î¾6ÃÀ Oœ'rÀ8AðáyÀ:c7ݼß@:<§P;'@¾¡žJÙB?¹ÑÓFäjù?Ò(ÝÚ;JY@Âl~®[È@ؐ$zß?ïÿA>8ÊÍ¿àzjÊy5v¿Þľ`xe¿ç§(bõ˜ž¿äQ¬šþ¿ïþi'O¦UNASNone3FGL J1457.6-6249?Ö¾9aª•?ÐNŽGDÒ?ä ãOp*µ?ÐNŽGDÒ?áJëÝþ#?Éôm8VK?Ýj)ÚD»?Éôm8VK?ßüøÞbK?µ{µîcöJ?àƒñÎÚ?µ{µîcöJ?è-êv"h'?§á'ŝ€?ÏHV'v]ø?§á'ŝ€?Æ«gø6Ýã?Á¤g†€?êU&òH‡?Á¤g†€?¶KG¯Ÿó?À5½ð´à?í6—
B?À5½ð´à?àA*"ãÔü?¶¼÷~½zh?ß}ªö8V?¶¼÷~½zh?ÄõŠ¾ùr?«æKŸ¡×'?êPÁ¤?«æKŸ¡×' MIXED4FGL J1501.6-5236¿²•3$yïÌ@g¥ßøù|À:fž—/\À;Š]«¬Á•@®šǦ@ßæՌŽï?Õ/`àëgÃ?ãwÛÈgã@{6½+o?ú"1Ó·¢™?ÆÛ˜ÜZ^?èSðlõÍ¿åõJÖ½ç¿îˆÍ¿ì³ß@ñ^¿ïýZØ®UNASNone?îçˆqAûg?©ºÚŒ÷÷R?¡‡x혐?©ºÚŒ÷÷R?ٕãË°±Ó?ÌÌ›êú?ã5'§?ÌÌ›êú?ì?úwk-?¢û´œÎY?¾/D¦›?¢û´œÎY?â³F|s)?²8ôk¶Ø%?ڙs­?²8ôk¶Ø%?ê·F¹Þð?ÅO»OÝôù?lj"å"A?ÅO»OÝôù?£Z>ڙ.´?±ƒÙ×Hè?îÊ\-1Å?±ƒÙ×Hè?àÖP¡?¸"ʶgÈ¡?ÞS_Õõâ½?¸"ʶgÈ¡?¨ÿ> ',?•h",çƒ?îp"¶M?•h",çƒ	MIXED4FGL J1502.2-5933¿ªâ4&úË¿è×z:XÁbÀ:6›X¶z{À<nšèN3@ìÖæ(ß@yn‡PÂ?Ó|_…?ïêÇß}( @·zâm©@÷½Ñ²9Ï¿ïò¶kawê?ïû|ã€m¿Ü‰¦qï0¥¿á?ÅGMƒ¿íûª€qªg¿èÃà•®UNASNone?ÙxqP¶b?̼S(­.ˆ?ãC±GW¤Ï?̼S(­.ˆ?×5óüUjY?ÊìBD.i[?äeÕJÓ?ÊìBD.i[?â•bRä-?³x~Pã?ÚÕ;Z7ó¦?³x~Pã?ÔæàmØ9?³¢%4Ô^?匏Éã??³¢%4Ô^?´ôØú?'5?ÄS÷Š æç?íadàïy?ÄS÷Š æç?£zn'EF¸?®ØY1šbß?îÈYæä?®ØY1šbß?¾íÅ.·'?ªN);Š0?ì?ÂGZ)?ªN);Š0? ]YrC0°?ù¦'Ó?îú*iƵ?ù¦'ÓMIXED4FGL J1502.6+0207?ïø¢áõ[•@Hï? §?uÀ;P¤J̓¬À<œ—w€j@ V"‰Š,ê?þ'ê–o ?ÐùùJ÷?ÃígaŽx?óy¡â=wZ?üjÔ²t[ò¿ïù™~Á¦ÿ?ïÕɕà§u?ï(¥:·‹ó¿åêa2Iÿ¿ÝŽè%Bڛ¿äƒÎSŒðUNASNone?ïúŠÕRú›?Rg€Á«6r?EÔªBHê6?Rg€Á«6r?ïªÓ"|V¾? úqÿ)sõ?…K7]z´›? úqÿ)sõ?ïP—Ç~я?'F1k§²?•í¶21?'F1k§²?ïòc_Jé?…†Ðò?Á³'^ÔÜ?…†Ðò?ïò®p–@?_ ©G}hD?Z£²ƒ"‰?_ ©G}hD?îZ󵳚f?¸â¦UÃ?ªPĤÆY§?¸â¦UÃ?ïLÿâùµ?•0_d¿õ?žv`È3]?•0_d¿õ?í$±Q¿Õ?¥eõ)»¥?¶ÚwN»ÛÖ?¥eõ)»¥AGN4FGL J1504.6+4343¿Ô™~aûã@MAtNƒÀ;±ôr{HÀ<æ¦qq@!:¾lâ¬?ûBr5§º?Þ%€W©4A?Á°ûàá'?ß¼[»g @^"'GA³?íîÃA³©¿ëZ=c7ݽ¿é•¢:Å?¹yÿöDëB¿é™RÀ—¿Ò½å=ÜÚaUNASNone?ïûX‹A£?A&ßÇ;ø5?BŸ†z¥%?A&ßÇ;ø5?ïóߢߵÕ?Z›=ñÄ?X@ºÇE9?Z›=ñÄ?ïǟzÈâÌ?€1—ÄÛ¦?|0B¼ŠÙ¼?€1—ÄÛ¦?ïèÙo"Úº?QЖÁ*?g&D©¥È?QЖÁ*?ïê
mñ0?oP‡¥MôT?eõç¥LŸ{?oP‡¥MôT?ïÔ²ˆÂ "?xô€®…ËÇ?u¦»†¢r»?xô€®…ËÇ?﫸:Í?†B]\Lh+?…ñEÝAÖ?†B]\Lh+?ï¨v)¹)?wÕÆÅȈÝ?…âu•(QË?wÕÆÅȈÝAGN4FGL J1505.1-5145¿êQDóœfË@WbØ<l˜À:P•,L%À;'(mÝS-@A—ȉG@R.»Õ-Ä?×ìe$?ãrl™†Nc@Æ.Z†^S?ý«è¨ˆË¿ä"œ!´/È¿ã)¨¥¦V¿â³CÕAæ¿ê…AÁÇ¿éèv¬.ǔ¿ïÎ0»"¦UNASNone?퉙KÀó¦?±ô(¯F?³³5£B=Q?±ô(¯F?å±æÀÏú?Ì?©X~qJ?Ԝ2~`
à?Ì?©X~qJ?ìu¿‡"ßK?¤%»ž£¯ø?¼RÃY«?¤%»ž£¯ø?í5e.¥QU?™ÁÉA/¨Ã?¶T֌OÕ?™ÁÉA/¨Ã?Ýá¶m(¼&?Ì3ÚS"G´?á$Ék¡í?Ì3ÚS"G´?¶èQ`æaÙ?¿s8SP–?í"õÓ¬:?¿s8SP–?ܹïìGͅ?¹µCKaÜ?á£	Ü=?¹µCKaÜ?ÖeړÀ?¿3Œä]?äͶw1 ?¿3Œä]MIXED4FGL J1505.3-5852?â·:I°€Ä¿Ø#dn•À8\ëÉVjÀ:ïLS•©@ÊþOPË@l»Ý'@/?ÐLÌamb?Ú@Z£'®@ Ÿ°4?ùB)Æ"¿Ù¼sƒ…[¿éyq%Ú¿æµ^ñýÞ¾¿æ~˜÷³*d¿íú'
‹þ¿ä8*lUNASNone?è|ï-¹?ÑOF¿'ˆ?ÏÂCI¾?ÑOF¿'ˆ?ä:Nî$¶C?Ëûq×DO?׋b#¶"z?Ëûq×DO?ߓm2æå°?¶=\ûÛ8?à6IfŒ(?¶=\ûÛ8?äúMçO?´AʺHÇ·?Öd0Åßb?´AʺHÇ·?Ù8×ÒºL˜?ÏǬ¶p®®?ãc"¢Ù´?ÏǬ¶p®®?»£Š;á5?Âiì¶TÃÚ?ìŽKŽ¸ƒÙ?Âiì¶TÃÚ?ÔÍ,íi?·Ÿ;•ls?å™xiž)K?·Ÿ;•ls?³—ôîrò?¤
H~N-˜?íbMŽ?¤
H~N-˜MIXED4FGL J1506.5-5708?ï÷døö?𻦺Œ¥À9*#²Œ¯¦À:ÈÃB	Ì@ƒÇaÓڈ@@ÝûÉ9š?ÑP¸_˜1?ÔÄÃÿž±@FGwÖ@°s#Ž$›?íçòpËD¿ßÁ‹›T.Ö¿äD8¿HB¿âë7@¿ì*í+&¿ïÿ·`)
UNASNone?ìø4àe
©?¹!ˆŽ·ñÒ?¸>Xý³y´?¹!ˆŽ·ñÒ?î¶5("?¬à!Ràø~?¯ÏԜ­}Û?¬à!Ràø~?æ¿ëÿܳd?³DèðÍe­?Ҁ(F™9?³DèðÍe­?í°àZü®o?'–
¼äÊ?²xý)ÒZ'?'–
¼äÊ?à´oØÍX…?ÈÀctíñ?ޗ NeNõ?ÈÀctíñ?ãíÖÂÄá?Ët9ÁJk<?Ø$Rzv=Ê?Ët9ÁJk<?Úpt}'Œk?¹Æz¦Û?âÇÅÁ79Ê?¹Æz¦Û?â¾üÅbö?²'s'˜?ڂu:Í?²'s'˜MIXED4FGL J1507.1-1901¿î)ôtþÑú@@©º^5?}À:Àh®?CÀ<)Táä·@ê+ÌâqO@œÃB	Ì?ÊK‰@[￲fCUë?è8)Âq)8@›oðRãÓ?í-$%y6M¿ê"`Ø\ù¿ì>â=ø¿Ä`‡êš"¿ïé¥J§Ãÿ¿Àø\È_UNASNone?ïô‡Ôu7»?\ü\sÔ§!?VðWx…Jt?\ü\sÔ§!?ïÒR¿"S¦?ƒr¹?ï?vÖ -X
?ƒr¹?ï?ï¤ÑPj%¹?`vÀ¨?†Ë«ìUÉÎ?`vÀ¨?ïòˆÐŒ?J?µÈs‡?Zî_¤ïM×?J?µÈs‡?ïñ
¶n]ù?aÇ×öAh?]ä"m{¡?aÇ×öAh?ïŽÇê¡?­"¾ü¤f?žn'c­s?­"¾ü¤f?ïwÒ>Ñ¡ô? ýb­#ƒ?'¸*ó+ƒ? ýb­#ƒ?ï<ù-³?×ÍÜÂ8I?˜pá)å§?×ÍÜÂ8IAGN4FGL J1507.9-6228e¿è¡Ktü	À
@$ À8èO,ý"À;`CނØ@"`¼x{?û÷Oݍå0?°h­é\Ð?Uö´9És~?îz£q+3?îã!øÎ2¿ÂM%²—¿àWÕ©ë u¿Ú~½ÀjhÔ¿ÖCÐú®ÝN¿Ó"j@ºˆUNASNone3FGL J1506.6-6219?ïø=Zö¾?HÂó?ØtL?O
"Ê'?HÂó?ØtL?ïrzÂ
?¥ßì–?'¾0 Þf»?¥ßì–?îä@+
½?™
=ÐØæ…?¡»ýLÀy¸?™
=ÐØæ…?î#´æ"·h?žJµjapÿ?­Ä±›$%}?žJµjapÿ?ïªÂ<ê°Ò?¬p?å?…Op´%¿‹?¬p?å?î~›o?»^­õ5?®ÖøÙs?»^­õ5?ï$	ïfÝ?–…É8ï?›~ÂÊòY?–…É8ï?é»ÿ´øè?·íW­w-D?É,_ÿ?·íW­w-DAGN4FGL J1508.4-4817?ŸI÷cÜðÈ@!)éBNYÀ:·o¿«|À<°}á­/@ˆmm–±@!#=ò©Ö?ØU-XþŸ?î┵.J–@ÁÀÊ`@ùï‰:Pß?îïŠ1FÉé¿á{À nŸñ¿ç³"âz´¿í³Y(B¿Ð†0[<'¬¿ïÿæŸÜ©ºUNASNone?ï<ŸxßBy?±°éyl-?˜lä°å?±°éyl-?íãÀA#5å?µ¯œîSSf?°áýöæP×?µ¯œîSSf?ê^qê?–ïæm·Ý_?§GY<ú`?–ïæm·Ý_?ïwE†ÇÛ?‹(øeº–€?Ÿ1Fþ³?‹(øeº–€?ïz"M¶?§ûý£¨À?žp¼jNßS?§ûý£¨À?Ý	Ë7mÌÚ?Òòd9C D?á{dI"?Òòd9C D?êF)b"¸?±t+ÛVü‡?ÆåËZu±!?±t+ÛVü‡?å¢H‹£Ñp?ÄS۟MŽ?Ô»nè¸]!?ÄS۟MŽMIXED4FGL J1510.1-5750?ïÅvgO?É7ÑÌÀ8àpØ°/ÞÀ:DÄ)B@ $ÀS @ZQ	Þ?Â*2	h?Ѐ{zõ"—@	—ZYè©¢@0oz¿ïÁ­)«Ë?ï'ÄþÍ%¿ã ®@š¤Ü¿åxÜö¼6¿êk7@7¿å®7¶O²ÆUNASNone3FGL J1510.2-5754?ٴ뉗ˆ?ÓF¹>òÑf?ã%Šq;4<?ÓF¹>òÑf?ä+³]B®Ú?Íä¢X"×?ר™Ez¢L?Íä¢X"×?ݲ…Ãù¿t?¸È"ÀNö?á&½ F?¸È"ÀNö?蝕 ?±ý+3ÔP¡?͋÷Ǚ©?±ý+3ÔP¡?³ÅßZŽ¯?¼¡y·Ñé?í‡^""lš?¼¡y·Ñé?Ãþ"ÙZ
?ȶ2/ìƁ?ë\7I©}?ȶ2/ìƁ?Å~®ˆá\ô?³—ƒ­"?ê T]ǨÃ?³—ƒ­"?½ªƒ)sJ?±ÇÙåÑ?ì\*¯šÑ—?±ÇÙåÑMIXED4FGL J1510.9+0551?î3é%ìâ@IM½ƒƒ­ŸÀ;IÝcpÀ<©7Ó«ä@ ¢§>H?þ7?öå?ÑWó;Ì^é?Ï
ŸÎ@ҘÀ¤ @¶ÙTD¥Ì¿ïùçýÕ®H?ïþY6Òúä¿Ø^m^'Rª¿âQ"ŒÂ¿×ÅÀÔqý¿ïüe"´UNASNone?ïމ!@0a?y}CÒYªô?p»o"7?y}CÒYªô?ï¦hR,{<? UV,ÚK?†eëj']? UV,ÚK?ïVÈ4>Ã?øv$c?•&ÿ^Ÿ'Ž?øv$c?ï"k¶Ì@?s½"ôaòÔ?‹%F8?s½"ôaòÔ?ïÌ¡Nç­?yöJ|.á?y¯Xù‰<?yöJ|.á?íʄPº¶'?¾Ð ‡›&?±«Ýz˜BD?¾Ð ‡›&?îÓÙnEØÒ?—W`‹œ[	?¢Âi~YÛ?—W`‹œ[	?ízÞ
o‡Ö?£ÃÄ$,' ?´)•_¨P?£ÃÄ$,' AGN4FGL J1511.2-5803?ï¼B‹Zy¿¯ù ?{À8u–†¿¢BÀ9Ó²ÊÃQ@ ´<[Ðá/@C{~% ?Ö_þ"/T×?ÃWÿJ?þm…É=?ÿÂ+[xv´?éu^C,P¿é‹^e¿äˆHn-Û¿êÒåëÃº¿åm$€½ÕŽ¿ê¬ÄÉ$¢UNASNone2FGL J1510.9-5808c?çƖ'Án}?ГÍ6ÿñg?ÐrÒú}#?ГÍ6ÿñg?éÐaOâQª?ÉÒH4ªµ(?ȾzÀv¹V?ÉÒH4ªµ(?ޒ2ÝwêÈ?¸4>9æD‡?à¶æ'D
œ?¸4>9æD‡?êÍ–D?²Z…Ýz?Ç°Ëͦï÷?²Z…Ýz?åœ@þL÷?ÐψE€µ?ÔÇ~f?ÐψE€µ?ÜU‰
I-Š?Ôá¨Â胞?áÕ;y[i;?Ôá¨Â胞?ÞÉт
©?¾¤ú1:z?à›>ú«q?¾¤ú1:z?Ão,º'¨?¹u*µœjÀ?ë$4ÑV?¹u*µœjÀMIXED4FGL J1513.0-3118¿åæÊ<
@6ƒõ@‰]À:Lm)ÏÀ<	Ä|œ2Ñ@ĐlIT]@Ý{~%ŸÍ?Ë®ýmS•?ÐÇ`&[^@Š#ÚМ@z6‡¦}?ë«6D_«a¿Ø	Žôúé@¿ä4߅·¿á'¼<[Ðá¿ïÿþ½à ¿?ï.°'kUNASNone?ïžÌŸçw¯?‰(pZ²³Y?ˆLØpè*?‰(pZ²³Y?ï_ru­?Ÿ<z¥O¿¸?"1±J\½?Ÿ<z¥O¿¸?îÒyyé{?"y¿ÓwÞI?¢Øh^ԚÎ?"y¿ÓwÞI?ï"ûÎö{?ràIÂóÛ\?ŠüAÑ?ràIÂóÛ\?î-°^'?ªhíž6]ö?­.oÔúß?ªhíž6]ö?ë2MŒƒd?ÄÚ+`cº?Ã7šÉÍòo?ÄÚ+`cº?灢åÑ3A?´ŠJ¡Wá»?Ðüº4]™}?´ŠJ¡Wá»?ì(\ð=a­?§Á›<C¥?¾½~òš?§Á›<C¥AGN4FGL J1513.7-1519?æÀè¾x~Ê@A¢´A»Œ3À:õª®d,À<§)¥÷ß@_JÄIpŒ?ÿ×E|Y?Évz° F\?ÙÞš@
•ZÀ?ö@›R}PbÄ¿ïþÃT~–?ïÿþªJl¿ÖÔ]Ofo¡¿Þ´Þ. |¿êÂf͓œ¿ïñ.á"ÚîUNASNone?ꔻ­i}?ÃmÞ	¶A?Å­ÁJZ?ÃmÞ	¶A?ìoØʀ?¸ÓSÒú‰?¼?×A¬?¸ÓSÒú‰?ìþŒÓ7Ÿÿ?£-oR\éò?¸™eÕ…?£-oR\éò?í¢Ö¯­4à?'·}Ÿûl?²éJƒr@?'·}Ÿûl?ä˝ÉeJn?È!hšô­?ÖhÄm5k$?È!hšô­?âÐÁ®-ä?ÐÁˆ®îH%?Ú^|£¥È7?ÐÁˆ®îH%?Ú¼õ"&è?ÂOtÉøÔ_?⡅=ìõŒ?ÂOtÉøÔ_?âSVÉ\Í-?¸–l;-®?ÛYRmFe¦?¸–l;-®MIXED4FGL J1514.0-6240¿×©æѬ
ÀÂ6ŸÏ=ÀÀ9Š»¬éØvÀ;6Û¿®×@S«šMÀ@WGC¸?Çê›ê¬²?ÉpNœ›+À?úzÞÞGH"@w9ÝÇEú¿ÓwÕd ¿ÖåoÛÛ£¿çUyC¸¼u¿ì"RÈú°¿Ôåî|b¿è©xŸNUNASNone3FGL J1513.8-6250c?ïø­͓`?PDÅÉÇÛ¬?MKäZ¥†ß?PDÅÉÇÛ¬?ïå-3óU*?|¯#\-¨?jÒÌ
­¢?|¯#\-¨?ïƒ0yÍÿÛ?†láïb"?3á{QýE?†láïb"?ïöåuBÕÆ?;†ÝJ
Ÿ?R5ð‡?;†ÝJ
Ÿ?ïÙ`­Æ^?x˜Cé›Ýê?sOÀ6+U,?x˜Cé›Ýê?ïE'¶õ—i?©M²	Iw?—[	$¼®å?©M²	Iw?íÀÔˆ»?¤'‹/	/?·Yù]Eøª?¤'‹/	/?^?€jXä÷©®?ŠœŠËܞ?€jXä÷©®AGN4FGL J1514.1-5805c?ìÑ6'6ž£¿Ò"á#
À8ìÆ)wÀ:I¶>ëÎ@ É•½@Ï8ÅCk?ÄWŠ@
\$?(žÒ
?Ñ(@;Œ'?째Ex§¿ï¬^BUÿ?ïIë`á—4¿áu¿¿èŒ'Jÿ†¿àé¦A¯(¿æ֒³ÌJÇUNASNone?é¯î¡¢–\?Ñ@øÿÁÓ?É@Eyu¦?Ñ@øÿÁÓ?í˜O1
¢?·Á•\á?³=†xs'ð?·Á•\á?ãÌž´?¸ð¸›Ç¯?ØgÀÃÿô—?¸ð¸›Ç¯?ía_€¸š?¡£ØæT?´õ{ú;4?¡£ØæT?à+ô­'s/?Õ9utÉM?ߨ¤Ý¡?Õ9utÉM?åC§,Ý·?ÓxŠ¨'6?Õyú±¦D'?ÓxŠ¨'6?åQ}K¸Ã´?ÀnáµDK?Õ]hŽx˜?ÀnáµDK?Û¢c]®˜?ÃÍùXؘ?â.ÎQ(³ö?ÃÍùXؘ>MIXED4FGL J1514.8+4448?Øòù}@L5BÙÏÀ9¾E	Œ³À<1¹[ÖÀl@
61u@­Ò^Ý?µ•¬O(Ý?ÅQî׶@Pó_ތé@ó̕ðB?ê_'Bd(Ÿ¿à¥è'
è¿âý ҈y¿æŽzí(8¿í-½R†`¿ÖNï|O0ëUNASNone3FGL J1514.8+4446?ïÌH]å ?'+
­ž'c?yÛò0ÀÜc?'+
­ž'c?ïì~01¡
?kŽ;6ø½©?cÏÑ£'?kŽ;6ø½©?î¡7:SãØ?— }óҞi?¥ìŒY	ô…?— }óҞi?ïÌ~&W`?]À/'Ï?yÀúY–ú?]À/'Ï?îՐÈ1)?£)Ÿ­!9J?¢¦ó8ò?£)Ÿ­!9J?ï»läɇ?Œß!,-W?$ƽÏèæ?Œß!,-W?ê<<ø•
Õ?³†-ú5Ñù?Ç«È¬?³†-ú5Ñù?ï3ÉS?"¦f%ÎÇ?Ÿ/ٚ79­?"¦f%ÎÇAGN4FGL J1515.5-4242¿é¹''Z@)Zb˧2ßÀ:F;ÉÚªÀ;óò#žjº@€àîË¥@lè–Vîú?ĉûVxÍ?±Â2"ý¨?êVjÀh:|@üžîJI?Ҍùx&'K¿ål….¨‰÷¿ê@ý‹±yŠ¿âàÓ«¿è|ûhÁŠy¿Ö²#~4c_UNASNone?ïó´Š-7h?YM˒ø""?X–ë4Þk?YM˒ø""?ïÀΘߖ?ˆ:±Öïi?˜³žà Ù?ˆ:±Öïi?﷛¾ÄK?~^hlÛ2‡?';ˆÝ.?~^hlÛ2‡?ïåÁ ü?O:i0R??j>sV–?O:i0R??ï…=‹?¨{?ÏÐgù²?Ž°:dµ?ÏÐgù²?î»'L¹Ü?´ºTÑZÔw?¯´MŒì0A?´ºTÑZÔw?îÝ¿3<°?™!Äoþ4?¢$Ðxþ?™!Äoþ4?îü´Üô•Ç?‹òêrîí±? 4²4&?ˆ?‹òêrîí±AGN4FGL J1515.6-5817c?ëôQR5µ¿á̓ ٔ[À8éŠÆ—ÿfÀ:'Œri©è@àØÏ›y?ÿ›¨g'¶?ÎçŽD%ô±?ßϏ_Yø?õ,+l•T?ÿ –H+gã?íu'}ô!¥¿äXYÐUî¿ç›Wã¿ãâæIu"Ø¿î]%uŽÛ¿ïîÞoŒÖUNASNone?âÉUQž¶Â?Ó}ïîÔ£J?ÚmU\'{?Ó}ïîÔ£J?ï,°ó°ïÕ?¤Y¾*{1W?šiáQ¡X?¤Y¾*{1W?áªÛHÄ®?µšDoö¦ô?ܪInwÆ¥?µšDoö¦ô?í켺—?"åȄ.F'?°ŸÇdÅ?"åȄ.F'?ä"êBJõ"?Ì)ñQLÆ?׺+{jØ?Ì)ñQLÆ?웱­Ã±?À1!Bi×?»"r"âx?À1!Bi×?ß{ŠMSùZ?¶³®-½aý?àB:ÙVS?¶³®-½aý?ç=Šá?´5Y@j?Ñûûׄê>?´5Y@j MIXED4FGL J1516.1-6429¿íYoÕGgÀyԀö4¥À:Asqç£éÀ;¹ë\ÚÌj@c¢fǵ@ë'Ü5ö\?Ôvóý=Wú?Ù%ñaËØ@R$ZR[í@…ÉêoJ?ï×"ÆÔeH¿àÛ
bY'l¿è÷ïÅöö¿æû	 :2+¿ïþ,@OÑO¿îôÔ#&vUNASNone?ïéO8f<º?]ºÑ€Cdâ?f°ÇhHæ'?]ºÑ€Cdâ?ï'ó¢ÏxN?'áoâŠ%?‹ƒO'ˆŠ?'áoâŠ%?ï¥ÝZõ«?ŽŒla1†%?KD[€''?ŽŒla1†%?ïs'¡¹p?pxgÝHó?'«Î\?pxgÝHó?ïÌ"$d…³?vÁ²GÔj§?yîíÓ<†y?vÁ²GÔj§?í^HùÃü?º{³ïJ?µ½ºW¡Ÿ?º{³ïJ?ì±<+2?©Ý­;>?¿v¦o|?©Ý­;>?덼Nò¤?£‡JGR?ÁËéÄ5q?£‡JGRAGN4FGL J1516.4-2640?퀠ÈѯN@9âÀÆ.MÀ;':ûÀ='ÛSxM@¦¢Ç•«M?ÿŽêéîEÃ?Ù¦û¢"T>?ïx?ânÂ@
UûÐÆW@4:¤ì‰¿íŸXàÁÌ>¿ë5ݜþ¨è?ÖȾË,d¿×wß4®]v¿ïÿëþ@bF?Ú>‰¨ŠÎ%UNASNone?ïv*ì½­ö?iÄÔI?':¢c"×I?iÄÔI?ïhhH,®N?Â³}Í3›?'òöÿ' E?Â³}Í3›?ì™o^¡dÙ?§GÔsíà?»4…
ôÙ9?§GÔsíà?î«5g&;?"![‰,}Ñ?¥N|¬ý8J?"![‰,}Ñ?íÏ®ÝT?¸U«µ?³y'‡Î"à?¸U«µ?슠T¹Ò?ÃWï{M~?»ªÿÕZ1q?ÃWï{M~?傂Ù0)á?¾Æp£g^ð?ÔúúMŸ¬>?¾Æp£g^ð?èâë΀è.?»nêaÇA?ÌtPÅü_H?»nêaÇAAGN4FGL J1517.7-4446¿ÀϘ¹þG@%w+#š8üÀ9Œ)s–БÀ;ÔÞ]	@³6	Qbs@ ò{²þÅ?»õÔ­ì·Ï?Á$HIDíp@hÚdeg@uó>#§¿Îú1^ò©«¿æp>Œ,ɍ¿ãï
¿[J)¿äÍLN+Í¿îM"¸aþ¿ï÷#M"MUNASNone3FGL J1517.6-4442?ïÃNJÒç?~³ŽosŽ?~:»D1?~³ŽosŽ?ï: 
?&º?Î|œ«a?˜»þ»ŠÄº?Î|œ«a?î©û@u‹?˜V:ˆâÉ+?¥`KúgUH?˜V:ˆâÉ+?ï&Ï´L'?¡Opؒ?›&	vm¼é?¡Opؒ?끥ËÅÕ?»šó5í!×?ÃáùhÐèª?»šó5í!×?éÀP ÈÅ?Ç µ'û®?Èþ¿|ñÜë?Ç µ'û®?éiþ1¯á–?³˜ûÐJ¤¢?ÊX9@y©?³˜ûÐJ¤¢?éÀþ>x¥r?±$žè/v2?Èüj8?±$žè/v2AGN4FGL J1517.9-5233¿è÷ÔeX@'Š^"3NÀ9….mє³À<
ÇÚÅ@…BüÔÒU?þpCÊZ+Æ?¾q)¸á—?ãssÊÒ÷‰@ —¨mqó@‡B¨œö?ïü'-ks?î"=ßßy"¿ÊͲûÀUE¿ãg¡yâÅ¿î—;»—ñ#¿íÇîÁ"4€UNASNone3FGL J1518.2-5232?"O¥;"¬ ?¦ëïs®?ï®Ájݳ>?¦ëïs®?´4ÙË1?¯&^ì>‡?íy|{ÀZ?¯&^ì>‡?«ds'Wn?œnÚ-…
?îI¸Í³Éé?œnÚ-…
?«l]K_¤Ö?"‡";u?îI:+J³?"‡";u?"6$Ïú?¼Å¿tAå?ï_îNôý?¼Å¿tAå?'hQn²8?"Â[s´`?ï¶_ªëŸ?"Â[s´`?‹MG{/D?x]¹)èíÑ?ï'ÉúƖc?x]¹)èíÑ?eÇÒ(ä 2?XaR§¥?ïê8-¡x?XaR§¥PSR4FGL J1519.7+6727¿ëISno§á@EòxžwNìÀ;5Ñü·v#À<ùm"X9@ $©iuÍ?üGÐ^QÄï?ÌJ?(ßÈ'?ϵшžI­@l6|"ÏU@t§^ÿò?ï˱^²<ÿ¿îz´0ô"'?ÁXée´º²¿×¾Nî÷ð¿éJO^âäf¿ãׅøÒåUNASNone?ïò–pm?RsR,§Ž´?ZӍì¹?RsR,§Ž´?ïàh!É˳?p<',M"—?o—Ýÿ:d?p<',M"—?ï¸Ût´?x Ú®sX°?É>˜Ü M?x Ú®sX°?ïàÓG˜Î?|«°{Þ?ƒåœ4P*?|«°{Þ?ïÝᲕ-?jD·UÉ`‰?q'£ÅI?jD·UÉ`‰?ïœX"Ê0?‰–yÈ{«Þ?ˆú)ÚÍt?‰–yÈ{«Þ?îùy=%æ?–¥)'"-I? hl*>¥ª?–¥)'"-I?íØ'Á1†?žE9\ŠH?·)>ÁösÔ?žE9\ŠHAGN4FGL J1520.9-3805?²xn@/÷ûH
ZÍÀ:}ke©¨À<#d"@‹ãJ<º@݊ú`"?¼+ö}ö%?°³'i#°?ñùYˆ1'I@¬ø¢¾†c?ïÿ™¾, ó¿à]d"Õ»¿é¿VŒÔ9¿âðP•CɃ¿à^Æz£4¿é9†3‹GÇUNASNone?ïù9F–Ñ?J,}ÄE?KçvbPY?J,}ÄE?ïÜqs=lü?šêÑÁe}?qÇFnX)?šêÑÁe}?ïÝo}
÷?wÈ==£Ž?qHA…Vüœ?wÈ==£Ž?ïò¦¿L?@­1j³?Z³Ä»¢Ø.?@­1j³?ïãèzÛÆî?lÖ×k6?l…ITو?lÖ×k6?ï&żÉ0?¦Ç9åÔۏ?›'H>¨?¦Ç9åÔۏ?ï›
Á鳧?ˆrÜ¯Øp?‰=OwÔ¦J?ˆrÜ¯Øp?ïµØ_ä'n?p]"…³ˆ®?'‰è
eÀ–?p]"…³ˆ®AGN4FGL J1521.5-8057c?ãåƒ2á
À3Ö/'4ø/À: ÃÄæNÀ<€ãÀ.@ÜaHÅ@¼@cÃb(?μz-È?ÃÏeÙM¹œ?öɊ=D
@™ÎwFÞ?ïó¤r:¯ÿ¿è</áoA¿èm`áAMþ¿ÖV¨ƒAh€¿ð?ï÷vG…UNASNone?ïÖ¶Qz	ö?¿¢H½ÿ˜?t¤×:	?¿¢H½ÿ˜?ïÞŒå^È?{"BÇ92Ñ?pý9Œ °7?{"BÇ92Ñ?ïn¤°Eyÿ?Š2œÙv?'+iò)V$?Š2œÙv?ïâDœxWf?WʅþéËÒ?m»c¨¤Ùÿ?WʅþéËÒ?ïž.Ã{¯?'39ue?~°è´ï"X?'39ue?ï`ÐD¦x$?¤â™n¤Ä?"å÷gÁ_z?¤â™n¤Ä?î?†u8?¡"ð‡÷aŸ?¬˜²‹Ov?¡"ð‡÷aŸ?·N?•ˆZ|Ú8t?¤–ď&ÿ?•ˆZ|Ú8t AGN4FGL J1525.7+1503¿îI঍@JOKD¢À:€øõJÀ<NúìšÈn@$¿÷t@öڜ™(?ʀµ^å?´C_Bå?çváfÃ.@V'Ìx"¿à'âLÒ¿êp'_ÀYø¿æ܀w¿ïÿ»6¢S|¿çlÊcfæ?ì A¾ç0üUNASNone?ïÿßGñ?@"éˆî<‰?=½h*Ð?@"éˆî<‰?ïõR(°'?a}³+à\b?U[®æS¤Ì?a}³+à\b?ïVa§ÿ|¼?'6l¸4ñA?•3Êü Ì?'6l¸4ñA?ïùFÙ5ïY?;İφÊ?J䚗¬§I?;İφÊ?ïÿÂÄúà?ê¾^ã]j>þ Ží'ß?ê¾^ã]j?ï¼H¾	æ^?'¥Ùc¡¥?€íÐyê–?'¥Ùc¡¥?žå¢ ?‹Ù%€@?Š_Ø?¸î?‹Ù%€@?ï² ׬O?y˜šN ûü?ƒwøŒ$°H?y˜šN ûüAGN4FGL J1526.3-4501¿îÁZ +üU@#XO	RÀ9äù8¶À;óé Àiè@;öófêp@ƦºêL:?¶z;°ZPY¿Œ•¢­Ù0w?ÕÁÔKFOp@'XŽó£?瘝N(ÿ¿åÁéå‡ó¿äâm©PÇ¿âø£JƒÄ¿â":‡»JÄ¿Îi{CÃ#VUNASNone3FGL J1526.3-4505?ïõäz,ZÁ?I÷5½IN?T7
?>?I÷5½IN?ïØSÿv?g±'ØÄ?sÖÄL?g±'ØÄ?ïØJ§C%o?t°<å¸Ò×?sÚ¬Mï(Å?t°<å¸Ò×?ïèT›ÉÛ½?PšÕº`Ä?g«dQ¡"ô?PšÕº`Ä?ïÙ®–?ƒ?ji\ág™ƒ?s(ò"4•?ji\ág™ƒ?ô<â?±ŠuLMڀ?¤—0»b*è?±ŠuLMڀ?Ðÿ¼?‡õûm.?‡Ü¹Y˜ò?‡õûm.?ï‰"¢†?z¼Ç'd™ð?·WP¼™?z¼Ç'd™ðAGN4FGL J1526.6-3810?éÐԞ¨L:@.Ž­=%$À:ŝ%Ü3À<°ùïDÆÙ@ÊI±Nìø@l ºŠ«?Ê0pÍ¥»?å}¦‰l$ì@‰¡vݬï@-hŸ¦£î?ïÕ'^éšc¿â鏰â‹{?½Á]'çüS¿æ[Ûâ¿¿êíò·B!
¿ïæfÁ«¨UNASNone3FGL J1527.0-3804?ÖÏÝX¤÷?ËGq\þL?ä˜|'S­…?ËGq\þL?Û
åN?Èü1½í?âzú~Ù?Èü1½í?àLñmɏ´?³,Ôñʸ??ßf$là˜?³,Ôñʸ??ãP[…•^T?¯ºÍÜA^ð?Ù_HôÕCX?¯ºÍÜA^ð?ºë°¾Ï3?¸O¤¾9,?좟iè&?¸O¤¾9,?®v6sF®?¶éuW£ñ?ôÐn?¶éuW£ñ?Ž¯'AÚ¸?«D?YÂã?ë\T6/‰R?«D?YÂã?ÁÓÿéQ4?©ÅAsTðÏ?뜫³?©ÅAsTðÏMIXED4FGL J1526.6-2743?ãH(zóf?@7®8ûÊZÀ:³*¸:n'À<¥Ãiv¼@Mâÿi,>@mæh3?̎BM'iÒ?ìq='‡­@ó'ªi@éR ‹Ñ/¿ß´[ÜõŽã¿Üυ
ñZ¿ÆGçà¤p¿äšyޓHÈ¿ïÿÞý¦ßR¿ç#î¢	ª¤UNASNone?Ñ[¼¯Q?Ç"*óÚ¾ä?çR!û¨Wx?Ç"*óÚ¾ä?Ö˜á°+#?ɟážãQì?äø³'êo?ɟážãQì?ÙÏy‹˜`?²À!O¨VB?ãC:3Ð?²À!O¨VB?ÚJry\ã?±‹Ths¨?âÚÆÀCQŽ?±‹Ths¨?gQ€¢¾?¥}¶¿8Gl?ïÅsßm0?¥}¶¿8Gl?®¹>;Ú3®?µUjÚX?v?îl!u?µUjÚX?v?²$kƒi~	?ž 3âf¯:?í»ri"ï?ž 3âf¯:?¥*—ÂF?'³îš×ü?î­^FvÜ?'³îš×üPSR4FGL J1527.3-3103?Úü4É$;@4ñá~4¹EÀ:åJrÀ<%1ðÃ@ú"\ñrŸ@Õ7ªÉ?Á·]ú²
Y¿"ÝLÌ·S>?Ô »¡×+@t³Pw¿ãÓÇÝúœ"¿ÐùW¥ƒh¿ìUŒŸ
FÖ¿á­IÿþR¿×Ōf«/ĿٙޣcòÄUNASNone?ïúûº(¸ä?<§—ÈEYb?D‡q7²?<§—ÈEYb?ïëŸaôU—?rˆE¿•í>?d`ž>"¡?rˆE¿•í>?ïáà|òc?mØË-ôX¥?n"(eô)?mØË-ôX¥?ïýë–o R?…{H)@?0£MÓ
âQ?…{H)@?ïÒ&Œöaà?v[óøàþê?vì¹eâ"ü?v[óøàþê?ïŠz½`s2?™â}hTŠî?aP–µ'ƒ?™â}hTŠî?ï Qx\vè?ˆ7ù¾è ?‡ë¡Û#Ö?ˆ7ù¾è ?ïíÝ[:cS?XW·®£Þ?b"¤æ˜ìœ?XW·®£ÞAGN4FGL J1527.8+1013¿ïdógÉÆf@HÁ´xB0ýÀ:께Çâ'À=ÏZ@Ѧ¦G}@dGšÉD'?ËãŸ6¼£?ïþå-7@''¡.¹Q@ÏUï˪c?ïöW	ÒÙ¿âô8ñ
¿¾Ôw»ù?ò¿êõ°»õ4¿ïþÈÈ[N¿íº(ðºßUNASNone?ÙìÁmÔD?ÐÙ4ë€R\?ã	ŸpÉÞ?ÐÙ4ë€R\?à¦Ip¿ä:?ÐZÐ5Œÿ­?Þ³m€7?ÐZÐ5Œÿ­?Þ»ñªŸÞ?³Îwˆ&ô?à¢*°q'?³Îwˆ&ô?Âè+@(AÆ?©¶ŒüI´v?ëEõ/õïŽ?©¶ŒüI´v?¿œÇ».Ùv?ƉˆtØ?ìgš$Ñ?ƉˆtØ?Âò{½»ŒÞ?Çá­sZ›?ëCa'È?Çá­sZ›?Äd±Ý™á?®•Áä¦?êæӈ ˆ?®•Áä¦?'fÖ滒;?…~|õ®tE?ïlÉI.?…~|õ®tEMIXED4FGL J1527.9-4943?íAÿ©ÃÞ<@š¬"¢ºÀ:N õCÀ;‰Ö,Çß'@"zvž˜@öuÂú»ó?Ϝâ#v&Î?Õ§IEbø@†NÜ%´@£E9›N?ïÿèã«6¿ë3!à¥q¿¿ç·€4mÆ¿å9ÞHT¿ïý6âjBê?Õ
‹ÄCç6UNASNone?ï^->Û?'»_T
®?"?z[":?'»_T
®?îÆùM?³xØ~OÉé?¯óžQG?³xØ~OÉé?íñææd´œ?™ õˆ¡²i?°pÈÎ$5 ?™ õˆ¡²i?ïg,´é×?€j3v	Q¤?œólÒa?€j3v	Q¤?î'5?–²£?¨Ý°6ùm=?­Œ¬"ÕÌ?¨Ý°6ùm=?ÝÒ51e'Í?Ð8M7?áågMl?Ð8M7?äû¦*1èì?·Ûê*´?Ö³«œ.'?·Ûê*´?æÚHd·~v?µÇ/;óD?ÒKo6'?µÇ/;óDMIXED4FGL J1528.4+2004?áD¸/ ›Z@J¿
=p£×À;møDøÀ<"ìˆ3@@ $¼ev|^@¢€…Ì];?Å«®o´¿¯ûÄÃ$=³?çžQYŽç@#+¿÷Q[?í¨)µ/ë¿î±
õ´M?œÄ1%oƒÏ¿ß¸ªŠ¿ãbr†/YŠ¿Ø#lÁŸG.UNASNone?ï¹ûe€Q8?´øš¤|8Å?&¨*Áù?´øš¤|8Å?ïòž\eËP?b]-µŠY?ZÃG¥ò?b]-µŠY?ïÜ.1Ê0?x®AT߯k?qèç)VOí?x®AT߯k?ïߌóC5?V	ñër-à?p9†]Îy?V	ñër-à?ïé{STÞ ?bcÛ£%Â?f"¬i)`3?bcÛ£%Â?ïÁBQփÒ?†jØ0Æ*ù?^Öö‡?†jØ0Æ*ù?ïÚ55kó?|îô%ìw²?ròåQ\JÐ?|îô%ìw²?ïQ',Ú÷?…¢ÅÜ*ð?•ÜMӅi/?…¢ÅÜ*ðAGN4FGL J1529.4-6027?æ>l'­õ¥À
ª'†VƶÀ:wP™u‡À;+;íìØ@cN€ÌC@yDàá6?Ì0_ïÉ|?â)ñk@«ýq°F"@ü¦
›I?ë–åõ'¾´?ä	Ñ¥y¡­¿åœ,ñВT¿éËÕ¡1¾i¿ëîjáö)½¿ï#ˆÕü÷UNASNone?é³"H̙î?Ãi4—?É3vÜ͘F?Ãi4—?æƒÎSŠ–œ?Æ\†|!	?ÒøcXêÒÇ?Æ\†|!	?é¤T¯/¥?«ü­Úv?Én¯CAk?«ü­Úv?é÷sU¦êT?¤8y¶)'?È"2©dV°?¤8y¶)'?Ò
6¯ù>?Æé¥J§Ãÿ?æùdý¨a?Æé¥J§Ãÿ?ÂÛµÅ?Ĥ)·Ö½ß?ë{‰¸¿O?Ĥ)·Ö½ß?Î;uPRí}?³ꡔ§Ò?èq"«ëD¡?³ꡔ§Ò?Îl"M,-°?¯ÔúP'?èdÞì´ô"?¯ÔúP'MIXED4FGL J1530.0-1522¿Øù8ƒ="@@V¤"‰—ÄÀ:°úìšÈnÀ<Ò¦*¡"@ÎÝÉl@žnëp&?˳+;-C?ãõÄ<ÛS@¶'ö @0W`¹ÿ?ïžæu¿±'	/(·"¿Þò¢¿æX~FVüf¿ïÿÿ&¦³?ïYÌ?SŒUNASNone?ãGS†:?ÍO4`t?ÙqYæó‹ö?ÍO4`t?䯠؎]7?ÍæŒàèQ|?Ö ¾NãE"?ÍæŒàèQ|?á
0ˆ¼…5?´*&fº6?Ýëžî†õ—?´*&fº6?é]‰©?1¢?®r@ó¼Úú?ʉÙ[9y?®r@ó¼Úú?Òt½tȲi?ÌÎcõ6½?æÅ¡E›¦Ë?ÌÎcõ6½?Áét<+Ä?Ź³ÍCâz?녢ðõú?Ź³ÍCâz?¿ëöfVÔ¬?©+•Ñ€>=?ì35%k?©+•Ñ€>=?Èp(À¾?´\"r7w]?éãÿùõÏÐ?´\"r7w]MIXED4FGL J1530.5+5850?ànŸŠ±@H
r!…‹ÆÀ;0mWoÈÀ<­
‡¶B@´×xÍFD@b??°ï÷?ÄzIÚÕ¿¨ï¥È /?à>¥ÂœÈ"@çòiÇ¿â"±?¨Œ|¿çº=³¿µ¿ék¥^¿ÿ¿Û"à?¿ïüc]j	?ïŒËà"©UNASNone?ïø¦Ÿ¼sc?hÔ؅wٗ?Me€ÇÔ¿?hÔ؅wٗ?ïôy#»?XÌ©€0UÍ?WÃ
o¢ú¿?XÌ©€0UÍ?ïÒe àC?l	pè-¤÷?vÍp	"4?l	pè-¤÷?ïôo¿'·?F33X`'™?W EÎ?F33X`'™?ïð×ïü¸ß?côš³ØZ?^P ^"A±?côš³ØZ??ÖI£7?ä¼ù2?õ?€Ø
zMÀ%?ä¼ù2?õ?ïÊT¢Tå?|ml',?z÷U¹$aO?|ml',?ïiÒ"x?‡'ð'U«Ï?'Å»»¡d?‡'ð'U«ÏAGN4FGL J1531.6+0406¿íËñ]OçI@F³åBåWÞÀ;VÔ"+¤À<‹Øž'&ß@
8=3<@Èáž)?ÎFacGM?ÃŒ¨šhw?öFl{S]u@W‡§£?ߪ_d"(?ïñgìxc¿¿çeà"œ¿ÜâÅB>ê¿ãžzߚ.ë¿ïÿÀ?ЀUNASNone?ïû-@<?C7|îÏ?CKúÏwß?C7|îÏ?ïæTux'.?uMùzN¬?i«Šh<j?uMùzN¬?ïÎèéÁ'Ê?zÙëTˆ~¥?x‹‹0l¦¿?zÙëTˆ~¥?ïÁÜÍ\%?cÖå¾W?™[Œgà?cÖå¾W?ïïÜÏN\Y?`wµkÃx?`#0ËÀ®j?`wµkÃx?ïNHl?£~ª+Âcƒ?–=\Víøl?£~ª+Âcƒ?ï'D´§Å?ŽÆ›ËÇ?nÓdâ¯?ŽÆ›ËÇ?îí'â¶Ý¼?'f •Tn?¡-ÑþoD?'f •TnAGN4FGL J1532.3-3857?ÞÞ4dô@+ù"pŠ¬—À:Ò«>݋aÀ</"Bð?™@عó¬4§@Iß9¶Úó?ʽ	¶74?°"ŽJ[?çÉ[ÉTrH?üùä]K?ïø¯^|ã¿är5<!ï>¿æBµâz‰¿â^06ÿpŽ¿å'Ë9NÖ'¿ï×G²JkUNASNone?ïúz=ŠD?C3¾R"¥G?FŸìÓ?C3¾R"¥G?ïšØÙþí?"¶š¨¯®{?‰IɃ´Xv?"¶š¨¯®{?ïÛJôª?sÜw¨Ã¯?rZ…Úbs%?sÜw¨Ã¯?ïή3"'Ë?Z7o‹/?x¨æJŞ¢?Z7o‹/?ï÷aYrsK?L©˜8a¥?Q=Lä©Ý?L©˜8a¥?íĆ\'å?¸$¾®Ú|?±ÛÍ Ó¶Ö?¸$¾®Ú|?ï²RS¨}?"w´+;#4?ƒkk2¦äç?"w´+;#4?îAF¤Ý£?'""®G?¦ûë™!ÁÊ?'""®GAGN4FGL J1532.9-0313?Çq¡|€È×@DR)AAé¯À;Z4ù»À<ʽé:ø@4ê˜d»@¢®Ñ9C?ÖTéf`‡)?ë6ˆ™"º@	 &5@H8}õÏ?ïå²af¢K¿å±ÏñD{Z?Ók—}µk¿ç¹¾!ä+c¿ïÿ¿h`;ª¿¸_ô‡PíUNASNone?ìéú×:þ?¾ŒN,ˆÊ?¸°)DÞ0–?¾ŒN,ˆÊ?êP¢QEN?ÆÛ×®Êz¯?ƽvºéÂÉ?ÆÛ×®Êz¯?ëU·€ùÿO?©Øïõ	Ɨ?©!üÅ?©Øïõ	Ɨ?àP~={>B?¶ˆ¾Ä»??ß_…	ƒ{?¶ˆ¾Ä»??ëVdšÖ§ä?ÆÔ¤‡‰KÄ?¦m"¥`o?ÆÔ¤‡‰KÄ?Ôó¯]-á?Òkvœ¥£Ï?å†(Qit?Òkvœ¥£Ï?刀@zè?¾Y<²7ö?ÔîÿÛ
0?¾Y<²7ö?À»õUgG?°V ©¹?ëѪ»f.?°V ©¹MIXED4FGL J1533.0-6239?ïÈ­øeÑÀ†¯f•À:w
)´.pÀ;¬;Oag#@ȯ+|/¦@È˛te-?ÛÜ:¾lâ¬?í:û@
þ
A¢a¿?þì¸"ÁE?ïâ, GÑ¿Ód~d‰íT¿ì&½F¿êÍì‡}7c¿ïÿØ]#Dž?ëÛu<Z#UNASNone?íÜõlL¸?¹ßÿ¬Œ?±SƒS¿Â?¹ßÿ¬Œ?å6)Pö'?ÍEy|ӆ?Փ­^þÝ?ÍEy|ӆ?ëbúH†¶?©33åû<?ÂtÝçý*?©33åû<?åjý–]ï?µ˜dØu63?Õ*ÓEÚ!?µ˜dØu63?è<þ|"?Ï&*<¥³ê?ϸ
­Š?Ï&*<¥³ê?½è݂/M?Åö©ü#µ?ì]äOº?Åö©ü#µ?ásý×lõ?¸ÅâÐÁºO?ÝQ&ò?¸ÅâÐÁºO?§Œò9K‰?œ¼†Ã#æ?î‡0ޚ)·?œ¼†Ã#æMIXED4FGL J1534.0-5232?í"í•Å$@QÔ=ÚV"À9—$tSÀ;NѼÖ_@¨a3÷~Q@f":Ì?½-ݳÏи?͛ƅ
ƒ@P +"?ø±\"±*¿î	\Ý°Ë?ïûPÙ6g›¿âÛÏ3¯Yõ¿ãðV+Ü¿èÏ}¶åû¿ê'úhçJ'UNASNone3FGL J1533.8-5231?êçn³´Db?ÃQÓQüÖ?ÄbE1.îw?ÃQÓQüÖ?ßɉv`Ú?Ë:[¦Cöû?à@;Dϓ?Ë:[¦Cöû?ìÈš6³¬?¤²K@k.?¹¿C.Jbœ?¤²K@k.?éN¡¶Ú®?§XB4£É?ÊÄõy$•G?§XB4£É?ÆI,RÞ
+?˜kܜùu?êm´ëH|µ?˜kܜùu?¨9ñJR?°é–^¶µ?î|`ë'Î?°é–^¶µ?×fI¨?¾¦TŠhE±?ä}Ìüó[,?¾¦TŠhE±?Åâ•)%õ?°¢ˆ«¿M?ê‡Zµ¶¹C?°¢ˆ«¿MMIXED4FGL J1534.3-3312?Ó꜍â"Â@2WÙÛ©¢À:ßØy©9JÀ<~Ú©.b@‡‰6õàl?ýL¹ñ'ö?Ñ»è#'?Ýp¥°@
E^³¾@oµ9Þ,?í`L•ÚȿڅKCuJ°¿Ö…ÜãÆ8‰¿Ú'}keª¿í²Ûe¿ïñn7@UNASNone?î§|Pˆƒ?¥áÆ°³O?¥ˆ:ôä9?¥áÆ°³O?îà'²¨;ü?¤Ž&"/Ae?¡öÔØõ6?¤Ž&"/Ae?í`_Â
ó?¢Šå~wéÁ?´ýïj?¢Šå~wéÁ?ïHג×?{º¦Š?å}³ý?{º¦Š?ì
Á£ñ-Í?·¥·‹¥™?¿'òàv'œ?·¥·‹¥™?ê@z"‰Í?Åñ
DO?ÆþíۘË?Åñ
DO?Þ6IôÑßÂ?Ã7ùƒ0˜ñ?àäÛ—?Ã7ùƒ0˜ñ?뛓ùéÝÌ?¢"i
Þê×?Á'°XˆÐ?¢"i
Þê×MIXED4FGL J1534.4-6719¿íeE«)ôÀ"ÞøH{šÀ:ª'ݽµÙÀ<9v+ÖG @zJ''?@(:6?ÎRçÃô*?ÒqÁä;~[@m^!ôFŽ?ù´à‡iÁ:?ïæ†è¼í?ëP›ÄDæ¿Ù?""Æ¿äHcUeb¿ïük 	ŠÃ¿ïÿÄ;-ÓxUNASNone?ïDŽT8ˆÕ?"¢LrSÂe?—n5ÎX?"¢LrSÂe?êÁh·}?À
—òiXM?Äú_'#î?À
—òiXM?íÂYdÜ^Ì?›"2Tïy(?±í4ÛBË?›"2Tïy(?éå!tfP¹?¦$ÊÐùK>?Èkz.f½?¦$ÊÐùK>?ìßL¬+?µò)F×?¿¹šž§?µò)F×?Ú͏/YÏ?Ð P¶6?â™8pèS?Ð P¶6?éÀ[(´mõ?¯ž#1¬w!?Èþ"].H,?¯ž#1¬w!?Õr瘢?µ¦€Žš]?åFž¿3¯?µ¦€Žš]MIXED4FGL J1534.7-5842¿æ'ÚÏ*0fÀRzÊÒÀ:¡s¥ê	ôÀ<–:º1¦@ 9ʆÌbo?þð– ÀÕH?Ò)0æQÙ?ïþ©Þá!n@kpüÂ]Þ?úô?Z2üW?îôÁrüvß¿è
þraF¿Ôsíw¿Ð¹PC9e§¿í²UB&Á
¿Úk ÀÀUNASNone?ÞFþ=+?Îê®{O_?à܀üa1k?Îê®{O_?ٜ8|À'N?Êß®("ƒ?ã1ãÁŸ¶Ù?Êß®("ƒ?ä<¨d¸'V?³ì±‰±ae?׆¯6ŽÝS?³ì±‰±ae?Óh=*Ì(?²-×c/£|?æKájòì?²-×c/£|?Î&R±õþA?ËÑguHñ$?èvkS'€p?ËÑguHñ$?©'ô{ëÈ?µ–~csœú?înÖંÔ?µ–~csœú?ÕVB.<?»¾imèø?åTÞèòáù?»¾imèø?¢Ê҈¹Ò"?'ÂwT?îÓRׂ!G?'ÂwTMIXED4FGL J1535.9+3743¿ã\1÷tŽ@KNã'áïÀ9瑳ò
tÀ<"âɎSë@–íÐÓl¤@™Ãیƒ1?µ
A\Õ?ÉiÊßaÏÔ@Ï8ÅCk@ǯPY?ïjøœ^oø¿âûµþ!s¿âOX}o—h¿ê«³AáKà¿çv"|#g
¿äk_ý–™UNASNone?ïÚ­ßæs×?r:ÞgoËù?r©Ô?r:ÞgoËù?ïñE"ÅN?c ©-``h?]tÚ;+x?c ©-``h?ïT
?]ï?ŽeINá6'?•~¸"ãÞ ?ŽeINá6'?ïêõ+»›?MÔ÷1Ioj?eô
º']"?MÔ÷1Ioj?ïŒZ(??'þ;qՌ7?Œà)dÂJ?'þ;qՌ7?ïÉ·Y'®?'×>"6éF?{$Sfmi?'×>"6éF?ìë–ÂàËî?¦v¢­Ü ?¸£Iég"?¦v¢­Ü ?¸ôÜ>?z¾Ûf{[¬?žQÓöüe?z¾Ûf{[¬AGN4FGL J1536.0-2729¿îƉ"Xï@6"9:´0õÀ:×ÌQ|ÊVÀ<I"G!þ@dš½."@¿]þ¸Ø#?ȑ²ZÙ.?©󼥸6?âȕз=@rƒ.H<Û¿á#bp7 €?ëì²ÍOÔ¿éj¡3–Û¿Õ6—;~Ü¿ëé[x̚x?'E¿&ñÜQUNASNone?ïøWŽ&'?J	ïOÄå?N¡ÊU=«j?J	ïOÄå?ïé'8©à?r[ÅX¦>?fØÇsM?r[ÅX¦>?ïÁ>V‰
?zW''%åÍ?`ñÄ=[$?zW''%åÍ?ïöçîÄÌ×?:'鉏©?R0"ÓÛ²?:'鉏©?ïÞEk«0?sùyîp?pÀ]:\4?sùyîp?ï~#…QtM?š
OAå0O?;ZøàV?š
OAå0O?ïª[j"ÍN?†×n/ÿS?…i%sÝu?†×n/ÿS?ïʝ´®©?mf; ûoÆ?z±%ú×÷I?mf; ûoÆAGN4FGL J1536.8-4327?â¼#±#è¬@#·ÃøôõÀ9­‹0JJ§À;¨#ÃS§G@¬º†¤ƒ@™åóí?ǵrþzCé?Ó4# Ál@€IÄo0:@/¡¨Ü­•?ï¸\Ó?­•¿ãšµùK°Ø¿ìpgÁ°9¿à™¬cû¿ïÿ݀y7$?ê|'œýÒ(UNASNone?ï®7Fõ?§Çp
 }c?"r."™u'?§Çp
 }c?ïBI­iþ? Ú¨ß[?—¶Ê_'À?? Ú¨ß[?$Ñ?˜:G¦<'>?§þ"K9á?˜:G¦<'>?ïOq_ò7?t´¢Opä˜?Œ,#¤"Ö^?t´¢Opä˜?ï(ݕ¶¥?¢ïü<Q?šü¤T(c[?¢ïü<Q?çZm	uu?ÍR–3ˆ™?ÑK%í?ÍR–3ˆ™?éÍ´Ÿ'ß?°»'Jœ"¦?ÈÉ-ƒÏ`"?°»'Jœ"¦?é¬p+69£?´WŒÇ¸¶¡?ÉN?S't?´WŒÇ¸¶¡AGN4FGL J1537.3-6110?Ù
^g¿VíÀåë`5ʽÀ:¼înÞ-À<5ÈÝT@9ג"­@N:Wê£?Ô#";9?æþ
·x§²@)@þÍÐÙ?ú¸6OL,?ïýi¸*~Y¿æ>
ÝS­§¿Øðh]a…¿èWJ*,¤¿îÓ6=ª¿ïȀâ¾|UNASNone?äÖkéKø@?ÈöefPê?ÖS(-h€?ÈöefPê?á}_±Ÿ?Ë3Î:Øe?ÝáÛ@œÂ?Ë3Î:Øe?腏íÚu?°g˜ÍcB?ÍëíÀH–-?°g˜ÍcB?☶þŒëê?­ì2Í—Ó?ÚΒæ(,?­ì2Í—Ó?×ùy·À]?Î	wëýr:?äC$~Ò?Î	wëýr:?¹s¦³yÞ?Âz÷?ìы)ƒô?Âz÷?Ñõ¦ã⛟?¶²'½¹%Ô?ç,Ž²1?¶²'½¹%Ô?¶ÂðUî%?Ÿ]ñ¤|ßj?í'¡õ]º›?Ÿ]ñ¤|ßjMIXED4FGL J1538.0-4638¿ìÉGß4$í@´À>IëÀ9¥£×àýÀ;V$fÖ@Mj¾È5@k#Â|ç²?ÄK9?ØÆÝ"/€@͌ƒ"_?÷΅Sç]È?ï"ßµ§í¿ärEb	àT¿æœ­äª9¿êðz¼^À€¿ïù¡¬'$¿ïïæ­H£UNASNone3FGL J1538.4-4656?䔨Y'?Çvã¬bI ?ÖÖ¯ïÇM²?Çvã¬bI ?Ì=*<~y?Å&ÏÖ9Š?èðµpÿ`b?Å&ÏÖ9Š?è"5"Á?­ËDË+Ï÷?Íï·)ï´ü?­ËDË+Ï÷?Õx‡m>"2?¯IÛnºÄ?åC¼I`µç?¯IÛnºÄ?̊tÅq0;?ÅúmI?èÝbΣ³ñ?ÅúmI?"ÖbB'k?›Ì­îmå?ïaLíÞ.8?›Ì­îmå?Ðú­ÁÕß?²Çî8#Õ??çñ©?²Çî8#Õ??‰cŽ'Q?u±L}#¾?ïšqÇSÍC?u±L}#¾MIXED4FGL J1538.2-6201?焻ž|,vÀåKþSýÀ:%™kvqÀ;&hI•u@dð9äRP@˜ þ?҆¨%M—c?ц^~e‹ ?úoŠfö¯?û:+õÒ*¿Õ<â^"o¼?ï£éIUпêoÞµ,¿çÒñ©ûçm¿é"µÏZEÇ¿ïó!ž¶9UNASNone?ïÂ=ñÁè‡?Æ?²Æ²?~á*
|p?Æ?²Æ²?íØK5ˆx	?²·ãÆ3aŸ?±=¦Uâ4?²·ãÆ3aŸ?îS:êU?–Ú"n¯Î?ªÎÌ_ÍA¨?–Ú"n¯Î?î"9ˆ.Y§?':pãC»ÿ?­Üg}öLŽ?':pãC»ÿ?ìyD
ÏZ?¾ÈQÛócî?¼5ߓ….?¾ÈQÛócî?ã]‰÷¡Gõ?Ñ؟q|U?ÙDì½p?Ñ؟q|U?ä"Þ¢?ãù?¶Â•h»?ÖØB»€8
?¶Â•h»?ß}Ä#äiT?½[`¤H?àAî
ËV?½[`¤HMIXED4FGL J1538.9+0425¿À)É¿žˆc@F
;:iÀ:Àß}©yÀ<dQüLY@E…x2Â@äG<Õs?Æ1'®ñp?·ßj‰5É?ððhGçö@(U+«u¿ïá) ¸FÙ?ïÓô©Š¨e¿àò¿¥œÝ¿êqðdx¿ÐgÔ$¯â±¿ïùÕ^kÆ"UNASNone?ïõdó—g?Tä)^ÂÞÚ?U6qº"=?Tä)^ÂÞÚ?ïã,ÉráZ?¤+Ã#=?lÓ6žü³?¤+Ã#=?ï•ÂT×Pg?†#'BOj?Šj͛'<?†#'BOj?ïØ%Uˆ?_P³«Lw7?sí{ÕΨ?_P³«Lw7?ï¹b҈"¤?€…nõB@#?§KQ@É!?€…nõB@#?ï->'•vþ?¨YR}aÐ?šX-´0X>?¨YR}aÐ?îì\@‰?˜îô,é?¡:;þym?˜îô,é?îþ
J9g³?'Foq$? [XùèÐ?'Foq$AGN4FGL J1539.1+1008?á3"ä}åÖ@G†Ð'}kfÀ:Ÿ9&A³À<WÛçl@3¡B/z@ÙÓËď?Å5 ÝD?±M…C÷&?èh¦è6µŸ?õËÂƹU?ïÿéà
v¿æùÕ
ãîR¿ëË>øcSŒ¿Ø7ÑþdõM¿çdßI® ¿ïÿæŸÜ©ºUNASNone?ïȀÞp}?ŽŒæOL;?{¿þ•—5w?ŽŒæOL;?ï»-Ý)?§¯Ícz¢?œšQ|(Ø?§¯Ícz¢?îì4(¦'P?–Zr뙑m?¡<½tºóú?–Zr뙑m?îª}ÖUÈÆ?Žb:ð‡`3?¥X"œ[A¤?Žb:ð‡`3?ïšNŠI
?"ýËÈ?õ8?‰l]~éȏ?"ýËÈ?õ8?é6£;j•?ËéF¾]ü¾?Ë%sW­?ËéF¾]ü¾?îÆx0#š?¡ÜõÒ¿$ú?®˜|!ßZ?¡ÜõÒ¿$ú?æ>.çt?¹
¶´æ?Ӄ¢1Ð?¹
¶´æAGN4FGL J1539.4-3323?ì'U&@1ˆ5ĊßÀ9(¼QT†jÀ<süQ×@ô$ª"N?øÿ0F祥?´þï3Ôî¯?ä']<ñøÖ@+‡_•'Í@æCÍ_CÝ¿ÓVºÂG¹?ïùgÁf?¾"–}/€¡¿ß';#l–¬¿íH>]2àþ¿ïéŸ
ç»UNASNone3FGL J1539.2-3324?a}íæ?qûðŽanè?ïî'äMj?qûðŽanè?³Â›é?²"*¥¯¢Q?퇽ª!@?²"*¥¯¢Q?°SÒZUa?ŸÕ/	}?íõ…´p›°?ŸÕ/	}?d+CŽ>Ùo?\b±í?ïëÔ¼|¿ç?\b±í?]IïT7—ø?TøkžKŒ?ïñ[S$"?TøkžKŒ?ŽZ©[èåÛ?•¯lã¯Ç–?Zg!?•¯lã¯Ç–?¼ÿ;+q•;?©PVòq?ì`š'ÍY?©PVòq>üq®
ò>ûFÁ•ÒçÐ?ïÿÇéÓv>ûFÁ•ÒçÐPSR4FGL J1541.2-5201?湫–àña@rkݞ¬(À:×t¼j~úÀ<"K<¤@"QÂ$}@o$ù´Œ?Ög½ž±†u?ïÿV¢N@
ï×hE@ÀUE+Ù"?ïñ¦ ¿ç¿ì3	ý¯Ã¨¿À'åbšÔØ¿áäñ`®—¿î0¡™¹¿ÏèŸ{°ÐmUNASNone?ç‡#"`£?ÈÄ«‰…?Ðñ¸Ù>¹é?ÈÄ«‰…?éDÜÔèá<?ÃókrîŸ?Ê쌬\{?ÃókrîŸ?ë¦sïæØ<?©!»|} ?Áf0@dŸ?©!»|} ?ç4šü<žc?²$|bÜV?іÊ†Ã9?²$|bÜV?àð¿ˆkžß?Îö2I±Ø]?Þ€ï(ÂA?Îö2I±Ø]?É|[â:l?ÇeüN®?é é|1e?ÇeüN®?Ûèn€wp?ÀíÂ
Ã?âþÈ¿ÄH?ÀíÂ
Ã?ÐEo轐'?·Á°bÝ?çÝH¡7·?·Á°bÝMIXED4FGL J1542.1-5901¿ïZ¤˜?XÀÙÖ»cýÀ9H.Ä8©•À:èºÃµÌÖ@…‡°@ìJÆͯK?Äwøõt¶¶?ÂXȃ'ðX?þcˆÕü÷?û")ÿ°z¿à¢R‡"Ä?ïÿRü&V¬¿æÆ×Tæb¿ë®\Ÿ=H¿îÏp;Ñg?ÝßNdgÌUNASNone3FGL J1542.4-5911?ï¿G®ja?€(æEr?€.fošÊ?€(æEr?ìܕå"ÿ"?¹$(Õìn?¹PÒüä?¹$(Õìn?ë§P¹«Ý¿?«ÛóWçLÊ?Áb½P‰?«ÛóWçLÊ?íBqi¤´? wÀøJ'o?·½ìtDæÞ? wÀøJ'o?êJ³'¥E?œ<ÊØù"?Æ×½1µjí?œ<ÊØù"?ÜÂîcí²˜?Ó¢+Db–´?ឈÎ	&´?Ó¢+Db–´?å=Í5Ûâ?¹\9Ð{ð÷?Մe"H:Æ?¹\9Ð{ð÷?Ӟ½Ÿ!1Ã?¾‰ƒ25B"?æ0¡0og?¾‰ƒ25B"MIXED4FGL J1543.1+4209?¹N÷­Č@J1a¡Û‡À;s¤ÎóÀ<ݜûMé˜@ .ÝNûÖ?ý¼\!iT?Ïíþ÷ÂD?ÌqG€r+A?ý™s,Û@	¸vk5X¿åõí!Öê]?í¦¡‡N¾?çV)Ø@ž¿ãh³¦Äz¿Ú®ÏÁsÓ6¿äÁœýýtUNASNone?ïþVÏ€?!Gbv?*"ó#'?!Gbv?ïòܙ§*?`—‹'Z˜?ZFÌã^á?`—‹'Z˜?ïÜóAfãË?kÍèäWp?q†_<ú™?kÍèäWp?ïíýÏN1f?JÖó³ÒJº?b0¡PyÂ?JÖó³ÒJº?ïýr¾Û¿Ñ?4Rz	–¦?4jW²?4Rz	–¦?ïҊ8ӆ$?zŒÊXr?µ?vºã•È?zŒÊXr?µ?ï´KõÝùV?ƒZã
…Å?'íìm?ƒZã
…Å?ïÙož"¡ ?d¨ˆ¤›¬¢?sH0¼ÿƒè?d¨ˆ¤›¬¢AGN4FGL J1543.4-5925¿îx(]lAÈÀ3ý»'!®À:žlwø_"À;°ñ~\ý1@hwê@$9Ãp,¹?ß#v\}¯X?æQ­Dq@•%t-Ï?ûÍ%7G?ïùrz(¿íUâ_±?€ó;#Ë¿ãéošÂŽ…¿ïýn?΢¿Ý
v[Q	ˆUNASNone?ëÇfë`O?Â} ûÉË¢?ÀâdR~ÁÁ?Â} ûÉË¢?çD{²o?Ç8}GÜì?Ñw÷›Á"?Ç8}GÜì?ë²Åd£™?¨>×;œ«u?ù4êmq?¨>×;œ«u?èN2vQ?«è›á!·n?ÎÅ¿5ú&¼?«è›á!·n?áò:ÐÐ?Ðátb6S?ÜçïŠ^`?Ðátb6S?Äâç«ËJl?È#ˆ×e¾1?êÇF
-e?È#ˆ×e¾1?á0ùl½îc?¼ô"»3GU?ݞ
&"#;?¼ô"»3GU?Ê{	­öf?³‡ˆŠëc?éa="'zæ?³‡ˆŠëcMIXED4FGL J1543.6-0244¿âªÄä÷ƒ@Cqà?pXÀ9òµ™ªaÀ<(P!Ô@$o¹Ì?@¥zxl"?ÂCK¯*ûV?Ûè]»Vƒ@`ûH
?önrtÈû¿á¤þ§R?ێÆ!7S¿áâP>ܵ¿éšïª/>¿î±±RóÂÛ¿ïÿ"	¶UNASNone3FGL J1543.5-0244?¾3q
s[?ß]Ľoô?ì9'Þ±ž?ß]Ľoô?ÖL¸š»­–?ϓÇNøÜ?äÙ£²¢)5?ϓÇNøÜ?Ö
'¦¹›J?±™.49Ñ/?äù7,£2[?±™.49Ñ/?Àzf5òˆÒ?¡ý'G²én?ëáfrƒ]Ì?¡ý'G²én?•-8Ɛµª?²"6²êY˜?ïV–9½»ã?²"6²êY˜?´Œ‹ÚB?Á¿u:-'#?ín|ÝÀ?Á¿u:-'#?±yÄ}°Ë?¡MØÓÍ?íÐÝçb‹w?¡MØÓÍ?zM…ŸË=?jz»&
i?ïËdô»2?jz»&
iPSR4FGL J1544.2-2554?åã)ÒÙ£—@6š€JœÜÀ9žµŒ>gDÀ<n5gÀÙ@"áÊà¹i@ÁµQà?»ï¨ïÍÙ?Øçz"0¤@ëOKD¢@Çÿ_¿ÛÒæÂAX¿Ô³7¥]È¿à`W=Ôvå¿è½¢B4­Ý¿íEK-û»Î¿ðUNASNone3FGL J1544.1-2555?¤f'¾jF`?²‰x5$Ô?ƒð J?²‰x5$Ô?Ò·1/"?ÆnÖRª?æô$ghnÿ?ÆnÖRª?ÏO;|'Ý?²uš,ц?è8¬1 ßI?²uš,ц?å"æ¢ÇüÀ?±D8ò?ÔÖ2ºp?±D8ò?‰PÊBº×Û?±¦Fx7Þ¹?×Ó?±¦Fx7Þ¹?¤—ɲQ|?§Êã'ã§?î¾vƒr™X?§Êã'ã§?šsìɳ?'•­òY2Ó?ï/_ÌnX"?'•­òY2Ó?¶÷/½V?¡f–̘P?í<á?Nþ?¡f–̘PMIXED4FGL J1544.9+3218?҇ŒËCÏ|@JÖÜGªÀ;Am
ÅUàÀ<Ç+w}@ ʛþ"Û!@%¸Që…?ÀˆÔº××ÿ³,†›»ý?ñ4XÖZë@ìU¿û??ïÿ?{@?¿íRŠ±ŸIÝ¿×M,Ù|Þ¿ßÖïEG²Ç¿Ê±"øu7¿æÒÎ8ݗUNASNone?ïøø*YÖò?DÕwÀ=W?LVohç¢?DÕwÀ=W?ïòÄóåj}?]%úþré?Zvè3Å|?]%úþré?ïåÛøŸõ?mÙ؞q*Ÿ?j$AÍàµ?mÙ؞q*Ÿ?ïìÈx²ÌÏ?JÀÌÜ
± ?c7‡~­¸?JÀÌÜ
± ?ïñKWtäŒ?XRäçëH?]iQM0§–?XRäçëH?ïÈnir½ë?''	ô¾·ð?{ÈË$ôޑ?''	ô¾·ð?ï۔D‰á…?{
ªå?r5ÝÑ½ ?{
ªå?ïÌž~°µ?wä{\È#?‹ÌØj¢¦­?wä{\È#AGN4FGL J1545.2-4553?Ô¤³ã
À'@O¿ZôBÀ9òóĈ[À;{<¤ËüÃ@U}£ôC@‹Äߘl?È9…‡¾Ð¶?Ԓ±êˆ@	¹JÚåª?ö³:9·±³?ï½!~TÛgå!I¿çši£1Èпå³À¶‰?¿ïþñ­VåÀ¿ïÔ'£]éUNASNone?쐍MÓ??¼É¡Væ<?¿Û{•'f?¼É¡Væ<?Øêïvùd?Ì~O—©¿?ãŠÿDƒN?Ì~O—©¿?ì7Ľ)l?£96ÌR¦?¾AÙê´¢?£96ÌR¦?áÆâžßîV?°¿€æx"?Ür:Â@#S?°¿€æx"?ã§%À¦E?ɼ/ÄFt?Ùò±´~³u?ɼ/ÄFt?¦ÊÀÚ%?¶£S§ëî…?î"Sþ@Ž?¶£S§ëî…?Û^1èÊ4?ºO€RÃÜ?âPçšñf?ºO€RÃÜ?¥"¦Oãצ?Ž±Â
Ú£?î­Õšô?Ž±Â
Ú£MIXED4FGL J1545.5+2839¿¾G;]5@IÜ1&éxÕÀ<£3vOÀ=Ñö®H@¾d`QÏV@ª×DÁ?ÙfÀ=ó*°?ïÿøÞ£Žæ@
š;e0ÜA@®ˆ7q†U?иw?Ò}ç?ïÿÁeÖt?´Â9JúO¿ì†×6&-¿ïú™Ž±ß¿ïÿý±q&´UNASNone?èœP}ÆÕ<?Îu7¸[¯1?͎¾ä«?Îu7¸[¯1?æþÙuŽ?Ë·K&û†?ÓüüMä?Ë·K&û†?èÐg.'Å?°°€4‡Šè?̾cGÍôë?°°€4‡Šè?×6Ö¹¾/Ú?µÐÕ®Ph?äd"£ è?µÐÕ®Ph?åk®È2'Ö?ÓÁŠ{çf?Õ(¢ošÜT?ÓÁŠ{çf?Ôº$«k?Ð1H&à>š?å¢íú*9K?Ð1H&à>š?Ûj_e§_ç?Â|Гù?âJÐM,P?Â|Гù?¸»µ}nÎf?¨ôé8¢º©?ìè‰Pm£?¨ôé8¢º©MIXED4FGL J1546.8-3244?×}´†YöÁ@1¢ß"xîÀ:ÀoB­úzÀ<m¿Ü#å@ r"õ@ÓðØï?€"º•Ë?«éÃþr`?ì8é‹It¾@+2ËÚ3"?²b× ôÓb?ïöѵ(k¿Û_9áÎÅ¿å¡Äÿú¢¿à¬Ô>±·¿ÚàÏ6iIUNASNone?ïý§æìç'?*ø*ÛqÏ?2ÀÆôÃV?*ø*ÛqÏ?ïã_Ù."ù?x¤®Ä¥Á-?l '	ԟ?x¤®Ä¥Á-?ïêòÓ­Í¿?l"d5äh?e
,†lPk?l"d5äh?ïø(Gò²å?6a§Éðž?O^ßêpÛ?6a§Éðž?ïûÎriT?:Ž<ôTr?@Æ6êmd?:Ž<ôTr?ïO"uÎ?£]⠀"ô?–
vð~+?£]⠀"ô?ïÝ;Æeæ ?|ì§ê/€A?qbÖ«—ü?|ì§ê/€A?ïâÃ"÷HC?]¼ºÂt1?m<Üܼ½a?]¼ºÂt1AGN4FGL J1547.4-4802¿äÿëBâ0j@o'½†,À9 MÞ°$ À;lÀh:{ý@+Ý~uÒ@ø1jWX?Ã=ÛØ®Wl?Ә•=×@äZÏYo?ÿlå#/Úä¿Ö#fmG¿á'u=™¾ƒ¿ç|OÁß3¿æN-Š|Æ$¿ïþè=k›Z¿ÀsiN¿UNASNone?åI¾X€ø?ÉiÈÊÎ^·?ÕlƒOÄþ?ÉiÈÊÎ^·?âþAµ	À&?Ì8uV2*Ž?Ú|•ì´?Ì8uV2*Ž?ê¤u»Ì|ù?¨ó.`e›e?Ån)Î?¨ó.`e›e?ë–ÁÓ5Ù?¡ÿ¦¾Æ$?Á¤ûˆ³(?¡ÿ¦¾Æ$?Щt&²56?Å·¼÷?ç«Eì¦åe?Å·¼÷?©Ê(?²ŠEí´Ÿ?înÆþgà ?²ŠEí´Ÿ?Ò+BÙÏ?´C¸[°³?æê^þ"v?´C¸[°³?ÇOüÏkZ?±L$gôn?ê,Ì%)}?±L$gônMIXED4FGL J1547.5-5130¿Ñê¡üax@÷RØҕÀ9C»€t.¦À:æ]	A@»¤"ÈŸA@ãO%AI?À8›Ñr?uကFv?¾=îß,‡?þ"jCk?ïþ•1U¢¿åX5`´ö—¿ë	¯Á¤$¸¿ÛŒ\å^>$¿ä8z?Œ1ý¿æ'zç&ë&UNASNone?ï߄M¾5?qªÖ±;Ǎ?p=Ù½Z?qªÖ±;Ǎ?ï¸hXGÙw?‹ø"À…°r?åéÞëZD?‹ø"À…°r?}£ªü?›}J¿ÿ?¦Wx&¡7D?›}J¿ÿ?ï¹rÊÍÄ?hsGó!0å?£MM>å×?hsGó!0å? ©~û?©Ç»v%Z´?§T}÷ÞL?©Ç»v%Z´?îç)ß`?¸ST¸Tu?®ÑcÆÇý?¸ST¸Tu?íÁBÁÑ7?£)3Iï½?±õéôÍ]F?£)3Iï½?íòë
Šj?œeÇ(IÕt?°h§8‡"¯?œeÇ(IÕtAGN4FGL J1547.9+0445?íÛhý«£@E5@N¤©À:ôéË
TîÀ<K¢î¬ñe@頚¿´`@½¶°_¯?Î˔¨î÷?{þì.¼Öà?¯ ^¶ï–?ýŒ Ãås?ïl….¨‰÷¿ÛÜŸBÑ¿á‹Çêüó¿á­.l$‰¿ä¢àj8'þ¿áB£þøCUNASNone?ï÷"n9C™?J•ÐWþSz?P÷$«^P?J•ÐWþSz?ïêI²{"?pËèàwy1?eä¶ꅂ?pËèàwy1?ïÒª¹ÉÝ&?wÛ}føz'?vª£'I4?wÛ}føz'?ï·ûî½&U?c9\à.=%?'A@,º?c9\à.=%?ïì®x	7G?aHŠ1—»?cQ‡¾o Ó?aHŠ1—»?ïo–¬26?œÃ ^6ö?'
*{wÇA?œÃ ^6ö?﹋FŌ<?"8ªZKP?.V"?"8ªZKP?î…,&pú`?'Œ09(¡§?§­=›"õ?'Œ09(¡§AGN4FGL J1548.1-4416?ïŠp1sóö@Þá"Å&æÀ:‡0áI\À;Ã?¼®q˜@ËT‹rj@å"Ùîô??ÈýGéΐF?á]ŸîGq@Mý&0ì1@)ÓøEÃ?ìr>
þ¿ã
n}Œ¿âÅ~ú±âf¿ê "Êý¿´¿ï÷2œ4~¿ï 0âvdUNASNone?ã;{¯ÂP?Èj¨µ–Ob?ى	ô {`?Èj¨µ–Ob?ÕضA^ß?ÈàK†Þxh?åü¤ßP'?ÈàK†Þxh?æ(Ýí§_?±à+Êü?Ó®D%ô±B?±à+Êü?â:à"BM
?­Ã±ègTo?ۊ>÷{eì?­Ã±ègTo?¸zƒ'?±?´Œ«€&?ìýЯt;*?´Œ«€&? ä¤©Éæ´?®¿ž£+¨?îñµµŒœå?®¿ž£+¨?Á†¬Ìõ?®{/ºŒ•?ëžTü~Ã?®{/ºŒ•?ª-Hì
³@?'q®—MQ&?î]+q?TÌ?'q®—MQ&MIXED4FGL J1548.3-2411?׸ߗL.Ï@7DIDíoÛÀ:†Ôt`úíÀ;ú—t%kÊ@·É³å±@"º\‡À?ÒE3{W3?Ì
/Ä=Ý?øÌs@i|›@j£·Õš¿ìFX^»Í ?íªü-¨…¿ãçŠ$Óõ¿çP tοê%~>Ê@+¿ïû?ÏLÚUNASNone?ï·Ø¿cm?ŠÏnì?'	ÐC½Ú˜?ŠÏnì?ï«.zoeq?'+´œ^®?…4aVh3É?'+´œ^®?ï;¥}R'?‹ÿ×m
S?˜‹P^Dâf?‹ÿ×m
S?ï³,mÈ
?gKО͏Ý?ƒ4ùh­"°?gKО͏Ý?îkCè¸Ñ?ª(·­A?©KÁs£ì?ª(·­A?íú'˜?»dL8pg?°(‹Í±¬¾?»dL8pg?éÉólÚÚé?²9‡CUx?ÈØ2L""]?²9‡CUx?íƲˈ˜Ú?Ÿ-¢TÈ#?±Êi¢ßR0?Ÿ-¢TÈ#AGN4FGL J1550.4-5354c?èU¿Xß®ë?ÌRó—罿À8}N€ÌCÀ9ú&	Ã@τ'Û9@ÊÄç%>?Ûqšânõ?Ì
>ðÛu@1bBë7@m%-O™?ïþ˜½?;?"¼ñ@'@¿èÇÚÄç%¿êë)CÆ(n¿àÞLÑë¿çÓÀì÷UNASNone?è"C›$"
?ѱܤÛ?Ͳñ"owÌ?ѱܤÛ?ëÆêSV¥d?ÀÅl{~P"?ÀäV²¥jn?ÀÅl{~P"?á%çºÜ+Ý?¹%&µ^a®?Ý´0ŠG¨F?¹%&µ^a®?ìæ*4­ö?¢q3ï=2?¸Î®_øƒÍ?¢q3ï=2?æ|ÙÒ»?Ï.\:NÁ•?ÓMÍúZ‹?Ï.\:NÁ•?Ú¥¾Kæā?Òm•€k†r?â­ ÚÀ?Òm•€k†r?ݓÕD•†:?¹e®ñʧ?á6]µ<ã?¹e®ñʧ?Ñ ŠÉ?ÂS²Æ?ç/º›zwô?ÂS²Æ<MIXED4FGL J1550.6+6027?æÔJUÊÉ@F‰"_ôöÀ:é5WСnÀ<ÒÝnÛî@ q¿ºëxß@³Y¼3øU?»__(R/¿³è‡UYh?ôý7Σg@¡Ë:¦o¿çxÂ
?©¢í\M¿ç›8 Z}û¿ÊžI—"ÆÔ¿ádãD–Í¿Ú4Ci\UUNASNone3FGL J1550.4+6027?ïþôXƯk?iž¿g±ë? ºtR&ÿo?iž¿g±ë?ïõ­Ÿ'^?VYö:Zª?Tä¥7-Òð?VYö:Zª?ïù/›ŠF?H$2îS\â?KóAŠßÍ?H$2îS\â?ïöº·Ôö›?5í×Âíó«?RŠMÓ»?5í×Âíó«?ïýù·ÞËt?(ê¾™<?02Ak£:?(ê¾™<?ï×­‡ÑßË?uE«µ—ÓN?t)<&.bs?uE«µ—ÓN?ïúÅ.®û<?W‡]±På_?DëDÅ¡q??W‡]±På_?ïÌ_ÿïäÕ?iƒ4»9³?yÐl-"?iƒ4»9³AGN4FGL J1551.3-4920¿ë1ò_8N@
x¡Ú°»À9҃pbh«À;/Ÿ(NÓ£@s˜.4›¾@P¤þQª?Í×yär…Ù?ÁNÔäÉBÕ?ô…Őe?ûÍQ¤ãNÄ?ïøM·†ê¿Þ3LÉn¯¿êâѼÖ_¿âhá}V¿ïø¸BÒ¨?ïtã׫MUNASNone?ïÕ敤m?…E³´ 5?u÷Òºm"?…E³´ 5?îž$G ê ?°""D>>?¦»'`ñû?°""D>>?îŽkÂ Ï?—^7ÌR²?§G!B>?—^7ÌR²?ïmûÐ4O,?{G´>î?'@…ôN°?{G´>î?íŸ/D*A?µÔd"ø‹?³…àÕt?µÔd"ø‹?ã èæ2úS?Ñ]ç·^Ñr?ؾ.3šY?Ñ]ç·^Ñr?é<·/E'?µ,u;ÜÉ?Ë«
#Béù?µ,u;ÜÉ?èsEø»EÄ?¶Ú7vèw?Î2èèî?¶Ú7vèwAGN4FGL J1551.7-4257?§ÅÊÁX5@!*2	g‡ÏÀ9ԗt%kÊÀ;‹Ûz¹×@ššÊA¥@Úú—
s?Ãóâû¸G°?¸¹Š¿zîx?ô,byqÛå@ªëhÄ9«¿è4ÛϲZ¿áâ~
ÇÚ¿éGimO¿åÕ¥¹b¿å"&"À¿ïÿÀ	oëJUNASNone?ïЍþþÃ?¬œwjäˆ?w¹Š'R?¬œwjäˆ?ïÀ3˜¢'€?ˆ
ٝÅÂ$?æ3ž8Ÿå?ˆ
ٝÅÂ$?ï·0×'?'¤.ȓJ×?'3Ê@V5…?'¤.ȓJ×?ïçݙp q?Pdä×íª?h"f«\nÿ?Pdä×íª?ïÑ34›ú-?|Lì<Ä*?wfeºAùU?|Lì<Ä*?í؞>fd…?¶Ç
Í¬?±;ƒW?¶Ç
Í¬?î¡ÖtÉß?œ¶p§Î^Ê?¥â˜°ÎZ?œ¶p§Î^Ê?îá%ùӅ?'å]ž]üõ?¡î
 bDz?'å]ž]üõAGN4FGL J1551.9-6015¿ïÿZ¬QŠÀÀYÓpóˆÀ:lù¹"á¤À<
øç
¶@š>C\¡@÷ÀOæÈ?ÔðÍÝîÞ?ïÿÿÃw@zæ ³iN@Þȇî¡^?ïôž"|å?Æö©j(€¿éo`
+Òí¿ïôQ«Ä>‰?é©£½^ð¦¿íMt']è¾UNASNone?뿸ˆƒWõ?ù¹Û¿•?ÁÝò ,?ù¹Û¿•?ëÙç»C@$?ÄC¬R-õ1?À˜aòÿo?ÄC¬R-õ1?ê'²ÌùöÚ?®éu£?Ça4Ì$˜?®éu£?ïh˜ ¨à?z>G~èÀ?'ìëâL÷ç?z>G~èÀ?äßP¼ŸÇË?Ð{ø´\=™?ÖA^†Àpj?Ð{ø´\=™?ÏnäÎ)?ÑtÒVñˬ?è$FúÌu ?ÑtÒVñˬ?ã HÆa?¼®˜YR¬ ?Ùþ¿nüs??¼®˜YR¬ ?ãí‰
Ž?Ðۜ%—?Ùôü$íää?Ðۜ%—MIXED4FGL J1553.8-5325e?ōÃ[?Ñ×r"eÀ6ˆËà=ÂÙÀ9‡‰Fe?@i9È£T@EüÁ‡m?ŸÊ
ª¸?»Q†'_8@¢l] l‡@©Ç "?ïÿÑa\w¿É_·
BÏ¿à-â@ÒX'¿âl"þª?"¿äžJÞÿâ-iànjAUNASNone3FGL J1554.4-5315c?ÑQ°Eqh?Ñ'ýrØ1?çW'ÝGKø?Ñ'ýrØ1?Áâd†åy?¹Û Ö?ë‡fÞ}Æ¢?¹Û Ö?ãÜò'?³°³Q\±?ØF±ûÿÚ?³°³Q\±?ÈtU2ñ"?­Õ+¥|$3?éâê›óC¸?­Õ+¥|$3?Þn÷ÕAÄ?ՉjÝn…š?àÈÿ"_?ՉjÝn…š?‰l Arsâ?X"ý¾Ö?ïšM~ìwÁ?X"ý¾Ö?é,à¨÷°{?²5Q$…§g?ËL}\!>?²5Q$…§g?}ßø»¢‰Ö?r®€Ñ·›J?ïÄ@–y\?r®€Ñ·›JMIXED4FGL J1554.2+2008¿áÿ/ÞȀ@Gäñ<îØÀ:³È±µRÀ<x úK‹@!x?×±W?ûQ¦&oÖ?ÁÆ£}sY?·KWí&ßh?÷zÀûÞ2P@I*-¦…¿ïÙ	Y¿ï@…3Ç-?ïùV˜"	]¿Õ\…ýZ‰8¿è•övêB)?ΗådsGUNASNone3FGL J1554.4+2010?ïø¦»§F½?NäP²Œ?Me·";?NäP²Œ?ïíÂ5ø"?k 	g?b=ÊL6?k 	g?ïËx§½Ú?|;íˆ5?zC¬Š/–ã?|;íˆ5?ïšÒô°Ê?y-?Õ?‰Ky	³q?y-?Õ?ï×YÈj´Ì?s}8AêK?tS±èj?s}8AêK?ï¸hÜãE_?'¤Õ.g"?åȾï˜@?'¤Õ.g"?ï•yæd½3?‹•¥oðæ£?Š¡†\ß^?‹•¥oðæ£?îð''ŒóÕ?•Ù6!+? ÷×ÙÄw¬?•Ù6!+AGN4FGL J1555.2+7103?ÅÕM™@Cš+<¼IÀ;
iŽÀ<å4W¡†@sgÇ9ï?þJÀ¾¡'?Òà!1H?ÞG^á™@h%ç}R?ý2xUQ@:¿ë64¥#:˜¿Ðô!:kH¿Þ¯_ÑvÖ¿åÑva†-¿ì´
(wîN¿ïüP}ÆÕ<UNASNone?ﰀ~žA?ƒVlB5"?ƒßàHREÇ?ƒVlB5"?î6`lÚÒ?°ôão»?¯Œ™øVkÜ?°ôão»?î}!$#1?˜nŀŠü?®Ø-ñ-hê?˜nŀŠü?ì¦Z˜ãøI?˜Zº:íÊp?ºÍ+8à=º?˜Zº:íÊp?ïOþk¢³?YwF†Â¿?– 2‹©¨?YwF†Â¿?äÊĚ=?̐ïlñD?Ökúv˅Ç?̐ïlñD?êF)¡?±¬{?)?Ç»þçYÉ~?±¬{?)?á/s@û"?·VDm Êï?Ý¡~÷ÿ?·VDm ÊïAGN4FGL J1556.4-6911¿å]¬R¦7"À'öº «qÀ:¶"ÿ®¡iÀ<qzØ
r¯@28EìžN@ðüõŠ?ÏcæÄŗN?ÙÙØN
O@¦ÝA‰?üŒcXÊÇ?Õ%ðál—?ïâàj8'þ¿Þ•¨sQ0t¿Úf('íמ 'ñ¿Ô×[œãUNASNone?ï~qB"ä? R:úñ±?1×ÅL›|? R:úñ±?íqY±C¦À?±@J·r)?´u2uâÉþ?±@J·r)?îÀm÷\÷?™²#@[kµ?¯Cùö{–?™²#@[kµ?ì±ô&ásÖ?–±U^<‡?ºp^ÈôaM?–±U^<‡?î¬UÖBº?¦W~sÑȅ?®U: i?¦W~sÑȅ?âñXîaO¯?ÍÎJL)?ÚN#=`¢?ÍÎJL)?êJØ	°œ¯?°eüH»Zµ?ÆԟÙ=C?°eüH»Zµ?à 
Ê¢6?µ¿¬sô?ß¿ëÆj»"?µ¿¬sôAGN4FGL J1556.8-5242c¿âú
·WßT?áG›*½™À8ÐÎ{ùu¢À:Qqâ›k@ž>õ3HW@ ~ÅؼÅ?ÍÅrûË
?ÖZÚÂïI@
Ødà
—?ü…¤DBz?ïó…hŠ-¿á{%oü^¿äÇ QºÞ¿éÓ¡Ó#ÿ¿ëTu£KÜ¿ïÝ{¦i‹µUNASNone?ä3$;ó;?ÓüÄ$\r?י·‰øŠ?ÓüÄ$\r?Ù'i|Ev?̄'Tžh?ãx>ËAÝE?̄'Tžh?ߦҋÜ?µÂݾ©Í?à,ðºð?µÂݾ©Í?àmþ!ûÊ´?´~Yè4Ïn?ß$¼j™?´~Yè4Ïn?ÇFížÃ=ò?Å39N'n¹?ê.D˜O0"?Å39N'n¹?£0À+Ÿž?²D\Xùõ?îÌóýN†?²D\Xùõ?È)@։äñ?±ªÐÀЩÌ?éõ¯Ê]†Ä?±ªÐÀЩÌ?žlH´–ùk?$"I+0?ïº2å?$"I+0=MIXED4FGL J1557.2+3822¿b[-ÎÉiÿ@HåæFñVÀ;ôÅjüZÀ=ž¬(—@ TÜY×`?ýZ&6Ën(?Ö6ë¤~O?ËÍ&#€7É?õ	:q@ÿxÍFD]?í :}Ti?Ô¢˜[V¿âå¹ÏD¿¹u‰€-+¿êÇøð?ŠÈ-UΓ¡UNASNone?ïÞŽÔæï?zŽ×LmB?põ8{o€¢?zŽ×LmB?ïél|øE™?iËܗ…??f"ƒ(¶¦ô?iËܗ…??ï}Éøî$?‡¦ê¾cù0?FÀé´'?‡¦ê¾cù0?ïÄ&å¿Yi?cwq%Z >?}ì<€I?cwq%Z >?ï ÇíƒÀX?Šôj6?‡Î¥ï!è?Šôj6?ï¡áÝç7˜?Žæ;*Dïk?‡‡ˆxs©ý?Žæ;*Dïk?îÏe•&?—>\Þ²Q?£	¯Ëòøª?—>\Þ²Q?îø¢˜?¿Þ–±? žcr?¿Þ–±AGN4FGL J1559.7-4518?݆>sV@nžÂÎFJÀ9¡Ä©èœ6À;ULf
 @¬3*úª@°#¾…â?ŹxǑúi?ŜçAm2³@ÅáõRþ?ù¢¾Úzà¿ìZÓÍ$á¿Ïߒâ›@8¿åÕí¨§c¿æÈÙ"E¥¿ìEÞ,ñ{¿ïúÿ?8$UNASNone?ï®­òŠ?ƒœY&‰Ä÷?"T¸"ú‹Œ?ƒœY&‰Ä÷?ì-é$qNw?ºØ[˜¤sŠ?¾¶ÜuŒI?ºØ[˜¤sŠ?î9"ÖÐËy?šì¢ºb?¬f•†ýo?šì¢ºb?íÿç2mN?'Tí7é`?°Æk¸?'Tí7é`?é—Zá3Gf?Á"T@§™?É¢"{2âg?Á"T@§™?ØCq—¥7?ѡݨð­/?ãÞG4-?e?ѡݨð­/?偁+8¾?¹ÅúÜ»¾n?ÔýÎý©Ž"?¹ÅúÜ»¾n?Þ£—(Qƒ?¾¢T¾ž5á?à®48k×??¾¢T¾ž5áMIXED4FGL J1600.4+0407¿Ôk=RhO@C¸ƒBÙÀ;	ð€0<À<€Ü…§tN@rX¡×«£?ÿd¢¬gÒw?Ïe»d°?ÈPIÄo0:?ùꁘñÓí@+´Ýí±t¿í‰Ú¿~°Š?ïÿVW$ª¿Ëú|]s¤¿Ú—8Á< Å¿ïÿÇËÜ?ïýjŸ>XUNASNone?ïìPÈðIT?dWùþ ?c¯7Nï{÷?dWùþ ?ïè4ÏÀr!?tÄ…o8›?gË0wçw.?tÄ…o8›?îåÑÌÍî?",q#;–?¡¢ã1w£#?",q#;–?ï϶¶'Tü?cþéCÁÇ?x$¤Æd¦?cþéCÁÇ?ïàä‰#w?p†cœˆ"?o€‡Z¨É?p†cœˆ"?ïT.æ'‰?¤|y
¸n?•z<¾¤â?¤|y
¸n?îk´UÔë!?œcw!3Q?©Dº¢±Mô?œcw!3Q?ï¤þŽ;?"՞¦ s?K|ƒÔž?"՞¦ sAGN4FGL J1602.0-4402¿ãÞ
yxr@-Õ
ˆïþÀ9Ú|#g
UÀ;h¦Bˆ@§*ѺÈ@_tÝÛ?Ã|(ÚêœÁ?—Ì—ó§,)?Ùhm
&Ú@úã(-ñ€?ïÒ6™A¿áÂlÁÊ:K¿ìY …F%¿ÓÐ.`æt¿¿êŠ?åHD¿å³JEžpUNASNone?ïÕ¯liµ¦?«QôU²!?u(IÀ&lï?«QôU²!?ïÞ4]w ë?|•א%?påÑY½N?|•א%?ïp(Æëå?-8kƒ(?'úç çÕ]?-8kƒ(?ïöäVþµ?93q]Ñ?R7TP÷UÃ?93q]Ñ?漢™…ø?ˆÑ×}ɽ?…YY¥9à?ˆÑ×}ɽ?îÖЁ받?±j1³<"?¢'÷â ÝJ?±j1³<"?îP˜6ù?¢$‹AŠz?ªöw
z'i?¢$‹AŠz?ïÐKjè	?gÈ:õ‹?wÚ1,Ok±?gÈ:õ‹AGN4FGL J1602.2+2305?åE8ãe.r@GoîN&ԀÀ:ß­z!.À<¯-‹S…¹@7ö'lO?ú½S,;d?ÌE}x%Ö~?åN•ÄøÂõ@˜u—5@ Žˆny?îE6̤¿é'ص8['?·SëåkÕ¿áçÁŲ§¿íB8¿d.~¿ïᐼ{UNASNone3FGL J1601.9+2306?§"ou8#N?´²
ԚK›?î†ÉƒB{?´²
ԚK›?Ü=Ký?Íڗùäæ}?ááz|Úz?Íڗùäæ}?ӗ,ù–`?±ÌFÉÞU?æ4iƒs´Ð?±ÌFÉÞU?Ñ6WTû…?¯iðJ¤ã?çräÔU'>?¯iðJ¤ã?©)|q²Î3?Áû9KN?îmh8×­?Áû9KN?ÀcÖoŸz?ÃÂk—J+j?ëç
d>¡?ÃÂk—J+j?ȕÄ-Ž?¯ÖÇöE?éڟ¸Žôœ?¯ÖÇöE?¨%/eM€Ÿ?™ØS`Àó?î}­	¸æf?™ØS`ÀóPSR4FGL J1603.0-4808?î&q26!ê@
ႁOùÀ9bžÕB½À:êæ0K!g@ìfOë$Ò@¿ãzŽ;˜?ÒLóc9‹<?Ôâ¿ù&È@Ù
By!T?ö>~À¨?ïûüР–ä¿âÝ|²ÙÀ¿éåïaLK¿è8«bnà¿íxrmæ¿~­C¼å›UNASNone?íO$Ù¾?º¡PÌe¹?µ†ß W%?º¡PÌe¹?à˜Æ܄#?Î)7.ÈóØ?ÞÎrF÷éº?Î)7.ÈóØ?éªs÷Ò¹?²
Ï[•?ÉV0 ·¹?²
Ï[•?åꝱg|Í?°Ï'ÔÙ¬?Ô*ĝ1f?°Ï'ÔÙ¬?äô×]I‡3?̉õ¾æ?ÖQElñ›?̉õ¾æ?§ù<
ï¤?´ª¡T© ?îŽl?!?´ª¡T© ?Ýb5
4£?½]€ÊÑÜ?áNåzåñ®?½]€ÊÑÜ?¬`W¶^ò?›Z^(%ú@?î9ÿšvÛ¡?›Z^(%ú@MIXED4FGL J1603.3-6010¿ÚNA‹)ƒ À̎ï¬.À9Í,Ñb¨À;ÿV?§µ¼@+~d	û?ýù™cé´d?ÁeFc¡?ÔÓXl¨ŸÇ@Ëï»@öצÅ|!?ïõ(5©/9¿}-©Ë.ÖÇ¿Ùä½ú¢É¿Úu»Ÿíq¿éõH·(ö™¿ë½¢yMUNASNone3FGL J1603.7-6011?×®7טéØ?Ís1½9(?ä(ä3‹?Ís1½9(?ߘÐ=g?È٪嶗?à3—áLzq?È٪嶗?àA+¡nz1?³ñ-Õ²A?ß}¨½#ž?³ñ-Õ²A?çŒ9À|B­?ªÖ-¡2q?ÐçŒz¦?ªÖ-¡2q?¥Ø‹ÁƇ¯?·ŸQS—9?î¢wDÒÕ?·ŸQS—9?¶JD½ÏLè?½"JåxâŒ?í6·hÛ?½"JåxâŒ?À ¿ïæP?°å¤‡þš?ë÷Ð l?°å¤‡þš?É}¤	xé?ªLnGÐ1?é¹ –ý¡Æ?ªLnGÐ1MIXED4FGL J1603.6-0451?ìóþBÌ¿r@@ÒÒ¡øã¬À:<‰œÌTÀ<
Ê©Üݼ@3»QzF@ÆH@áqŸ?Å|ˆÑm?¸­z÷íâÇ?ò9,qx@fº¾'â?ҋ¢cAÄ¿ä'|^ö/¿ä‰}+¤É¿æ•ò—Ÿï¿èÒŠÝ>4¿ïýýâŽlUNASNone?ïq"ô_Ғ?±,[TÜȐ?'Ïat­¶?±,[TÜȐ?ïÌÖek®?ƒ`®!V3?yö¾+àá?ƒ`®!V3?ïN–¾ˆ*?­ð¾™ƒI?–-=Ï2­?­ð¾™ƒI?ïSÈ&Rƒ?w@¯½ÞJ‹?•÷Æ®?w@¯½ÞJ‹?îjÃU"
?¤ÅÍã¤ßÜ?©SÇÈï1?¤ÅÍã¤ßÜ?îa?³Š'äò ?©îv,çp?³Š'äò ?î;~O?¡4©YDÓ?®£$Ö9	?¡4©YDÓ?ìb´€$Ó?¡u÷'›*?¿œê[þÙd?¡u÷'›*AGN4FGL J1604.4-4927?à#‰A)7~@Àù²%À9:×ÑÍnÀ:¡²okÉ@18qÜf@26~AN?É
¢Gèø?Ӑ±þë-
@gȖÝ@=¨ø1TŒ?ïáâ"o?îƦ!è2.¿ãZ-þ•ò›¿èòbüO¿íRC™²Ä
¿ïýÚá¸lCUNASNone?ê°]ð?Ū%ÿ7Õ?ÇÁ>ˆ?ÃÔ?Ū%ÿ7Õ?åÄîì~»>?ÉYŽUf?Ôv"'‰ƒ?ÉYŽUf?å†d
0?²,ïmÓÆ{?Ôó7õåŸ×?²,ïmÓÆ{?꜇žö?©¯Q¹z??ōãń%‹?©¯Q¹z??ÝÛ{¿q£?ÌݍJ5?áB G.y?ÌݍJ5?Åï:äñ?Ççs¹'?ê";qxÆÄ?Ççs¹'?Õ$Àº˜?·xó´ïö?åmŸðö¢´?·xó´ïö?ÌXXu{Æå?¶ršÀúËR?èééâ¡G?¶ršÀúËRMIXED4FGL J1606.2-4602?¹%ˆP3-±@7 ÜïYÀÀ9üÒhAÀ;'²køvŸ@‡,ÓH@éi]'¬?×s]á~?ïÿ®2D¡@öà鳍@˗P=Ê?ïäžvx¿Ú'¿ó v¿é¥ø']<ò¿ïÿB€X*¿èt—1š­¿éØAŠäËUNASNone?äÿ¶ñï?К›¡Žª?Öޒ!Ê?К›¡Žª?ÕcMý¹Ô£?ËÜø֍bK?åNY#¯?ËÜø֍bK?è\l\Aì?°3ƒ§·6?ΎNŽû¨O?°3ƒ§·6?ÚbþNÇZ¿?µ¡¨Q…h;?â΀؜R ?µ¡¨Q…h;?Ýž‰då?ÓL~±"j¹?ás0»M@?ÓL~±"j¹?™Ôˆ$Ë:?§ò£	Õ£?ï1[¿eÓf?§ò£	Õ£?ÝáqIç?º/ɗõ:æ?á~yÇ[
?º/ɗõ:æ?"U짦?ŒA	%;Ðp?ï_Ÿ%'_s?ŒA	%;Ðp	MIXED4FGL J1608.4+0055?ï²É24@Bà~ZxòÀ:"€žP¸À<<g/ºï@lpÕ«Æ@)´Â&?Á">ï)?€» ¹Lé?ÁDŸ—4@Ì}EPC¿¦~ƒœ4Ý
¿áÄÁ/à˜\¿å?ÐÐgŒ¿é-=%$}¿ïˆ3
‡¶?ë2'¸#È\UNASNone?ïãL(€/n?M"äÕSm?l³×NV2e?M"äÕSm?ïê†úŽ.µ?q{ò`gÃ?ey«Šº³?q{ò`gÃ?ïbú4R'?‹鸞ÛC?" ¹|­Å?‹鸞ÛC?ïÑZÈoè=?cHjòÑ?wR›¯þÆ?cHjòÑ?ïRʵ›Wà?'lÕĬ½š?•¦©EµÌ?'lÕĬ½š?ïV^ÿ>äí?£,P6¹?•4 D*d?£,P6¹?ïΩ4°û?"ú–É*Œä?œ&*ÕúD–?"ú–É*Œä?î³YÀ™Ò?"ˆ3%?¤Ên5®0×?"ˆ3%AGN4FGL J1608.8-4803?ìõUš;U@"ÛÄ·UÀ9"¾®&˜À:¸Gõb@ÎfæÀ@—G½-óX@ëMý¹Ô£?ߛ9ÂC†è@ù¾$"]??úܔîZ¿àû	á€8¿ãr;ò•í¿çiŒöóçÄ¿ï8ÜÀ_×?ÕH߂\L¿ïù"–,ýUNASNone2FGL J1610.1-4808?í‡ÑÆÞ?ÆèÖÎXh!?·ÛÁr=Ď?ÆèÖÎXh!?áà<áæB?ØZ]™Ž1?Ü?†<3{Ç?ØZ]™Ž1?å²±J1ÉÉ?¶á[fbr?Ԛkœln?¶á[fbr?êÔ9ˆaãË?ËnŸZxÇg?įÞxpÕ?ËnŸZxÇg?åxèlš³?Óc'¾-D(?Õ/é&ʚ?Óc'¾-D(?ƗÀÀ=áý?Òo•Â¨Z?êZÏð‡?Òo•Â¨Z?Þo¶#p?À5Exv›?àÈs¤ðîH?À5Exv›?ÍLv´8#?Ö÷.ÜG¥?è¬âxÒñ÷?Ö÷.ÜG¥MIXED4FGL J1609.3-4326¿ì¤r‡ÿ5@c%}h
«À9ËǐíùÀ;[¦?šIÃ@	àÀõ~@ɎSë9Ÿ?øS"¢Ù´?ÚMú^ÖO@ŊžT~@zYWµ¯?ïÕ½Àƒ¿éÄ#°ß0}¿èb­ß¡»§¿çÜ$X¤ÜÄ¿ìFö£–¿—ß~øzòÝUNASNone?Ëø<?¹ŽIÒ'ã?¤$^øJE?¹ŽIÒ'ã?îçù•q…˜?¬Ù‡¼¿'å?¡€f©Ã}?¬Ù‡¼¿'å?íKéFkÄ?¢¥ºnŽCž?µ µÏ|¡ß?¢¥ºnŽCž?ïtyN w?€È—5Ì¢©?'pÖ&ɵš?€È—5Ì¢©?î6Ni«¦s?µðWÎ?Šý?¬›cÊØ?µðWÎ?Šý?ç>È+
°ÿ?Ñ·eO?тo©äž?Ñ·eO?èá§?I–ø?²Lá")¢?ÌycÙ¤!?²Lá")¢?æÛA®ä©?É&=ñ?ÒI|¢à6®?É&=ñ	AGN4FGL J1609.6-4837?ï­ú‡˜@rï
åÀ9Ú'(böÀ:•V|
—˜@wh&"ùú@FxõŽ?Í2×XA	¶?д䣮…@ÆeÊÞ@[¤ÍOA¿ëLA³Ù?ïŸá§Oe¿çì×Ï_ND¿ë%5C®«¿äj)i…Õ—¿ïÿÿÊPËUNASNone?îBÐ#[?·'Úl*r0?®+Òü¼U?·'Úl*r0?è0Ë<ÔÈ?Æzý—oó®?Ï?ŒÓ¬â?Æzý—oó®?ç™Ô$Yüv?²áˆs©x?ÐÌW·L?²áˆs©x?ìà³;¬('? ƒàé?¸úf#®ì? ƒàé?ê²Ð³ûßN?³Ñ-Q?Å4½0'É?³Ñ-Q?È5›@@j‡?ÉÄatË???éò™/ïå^?ÉÄatË???àlZ{nÞ?¸ó¹\Uá÷?ß'K	#üE?¸ó¹\Uá÷?ÐÌe‹l|¢?¾-V7*?ç™Í:IÁ¯?¾-V7*MIXED4FGL J1610.3-5154c¿Úž—Ùò¿Í@,ÀÓÀ8wSŸºEÀ:óøŠÀ¹@tœ…\JÚ@z–¹ëH¹?Å54?LÇ?×6a7R}@jaâs'?ᝄƒ:'¿îìñe2‰À?ïòË.g˜¿áõ³Á
&¿è§ØVmÊß¿íûW>«6z¿ïüD¿L±‰UNASNone?݂E¯â†H?֞¨bÆYý?á>Ý(¼Ü?֞¨bÆYý?¾"dțS?¹zﶣîò?ì;³f알?¹zﶣîò?҈,ãý"¿?µº¼—àè?æ»éŽ= ?µº¼—àè?–ðŒ
3z?'Åë'Ðɧ?ïH{Ÿ¼&?'Åë'Ðɧ?¿±Û.åF?ÑPäÅ£?ìIĚ#W?ÑPäÅ£?‰OœqüvÒ?B~lÑìE?ïšÁŽoä?B~lÑìE?¥tÿj•?—‹½Át²?ðNß?—‹½Át²?.ägñW?$'^ßeBv?ïþÏ8?$'^ßeBv%PSR4FGL J1611.6-6013?Ó½8Ò{ÛÀ»<ĬlÛÀ:ïÁÄ[À;É°pçÊ@Ö)ax@@•sd{ª›?Ðã`¸vÔ?Ö£²A†24@hXJb?õq	̆+?ïû?¤Á¿ëž'ŒŒÁ¿ÚÝFA­ÊS¿æ¾Q€ž¡¿ëV8!ï¿ïøžý†¨üUNASNone?îæ€ë!÷w? ×YÝØ=?¡—ñN¼o•? ×YÝØ=?ëŸ:ÊΒA?½ÙéÀÎg?ÁƒÔŶû?½ÙéÀÎg?ìœ1ûê`u?£ku7(z?»p ¬üV?£ku7(z?ë-êÊõÃL? TNaé?ÃHTÔ(òÏ? TNaé?ébª;Ÿ¶?Áç¬ÄfZ?ËæuW)?Áç¬ÄfZ?Õк@
å•?ÏÏÖ4³¤?å¢ßú6?ÏÏÖ4³¤?äáÕãKê9?¶ÇÎÊΦß?Ö<T9h+?¶ÇÎÊΦß?։÷Ö?´‰ÚêÛ?ä»ö~•?´‰ÚêÛMIXED4FGL J1611.9-5125c?µÜÕB7/¿¢ÀòyÌéÀ8$¹ØÔBÀ9Œûµîcö@xOE¤~@ŠQã!¢è?Âô`$-ó?×ÅäêÑ@"8]>Ÿx@\ÏRc$=¿Ï2¾°Õ?¬£"Šùï¿ãW榒¦`¿é'š¡×U½¿îûs®çŠ¿ïÿcøÍܗUNASNone?À
}÷?Ék&ÒÛ7Q?ëÜ»ý`'?Ék&ÒÛ7Q?āÕ?¼ü^AÌ ?êߊ"}ӕ?¼ü^AÌ ?Ëúxc‹b?³Ø$+[âû?éaç'{?³Ø$+[âû?ɗoÂIë?²'Í<ròÈ?éš$m ?²'Í<ròÈ?²Î›@ÿØ?ÍJ¥=šGó?í¦,˜%?ÍJ¥=šGó?‹¬‹ä¥0§?Ppšl´Q?ï'MÐmk=?Ppšl´Q?š4+^[2´?Ø£¹×j?ï.^¥Qޚ?Ø£¹×j?hæÒU¹w?aµFE¤þ?ïçú‹ÿ?aµFE¤þ4PSR4FGL J1612.1+1407¿í:åî»,@DÍÇ%ÃÞèÀ:†w-^À<ÂÛpÔ~r@Ü0Âë?ú†ØF}'Ó?ÇëX¦4]?æö·¢CC@¾1)?÷ä‡ÑÆÞ¿ïÿþøþ"?ïÿk»9ýR?»"òm›9¿âòq׳°œ¿ìÐ5½Q.Ç¿ïøœ>9¡ŒUNASNone3FGL J1611.9+1404?œR#©Ìn?¼ú¹¸%©e?ï-nðp?¼ú¹¸%©e?Ðóß×|ºL?ÊB˜áÏ?ç†A¢Ú?ÊB˜áÏ?ÏÓòÝúéã?¯Ô9'fÝ>?èHE‡?¯Ô9'fÝ>?«"È¥øVü?'ÝƳòÐ?îMÓu»÷p?'ÝƳòÐ?¹`3P_J?ÑcÔÆk^É?ìÓù–R?ÑcÔÆk^É?²;^c@IÐ?»æúܐË?í¸"3S>–?»æúܐË?¹\& WË?§…œ‰#"Þ?ìÔ{<Ü÷?§…œ‰#"Þ?ql¹WH=?e:vú*y‹?ïÝ&C±?e:vú*y‹PSR4FGL J1612.1-4526¿ìªGo]ä@5àqÅ?:À:"Ëùh6JÀ;ffÓs¯û@geÀy,g@Ý`#Up?Ùª\²½­?âH«4̐g@dϝ,@ 4¸ïJP?îÂOpV¿ä?3ÞLQ¿á'ˆô'¿é¹È®Zÿ¿ïý¸AûM¿ä²@Äì-»UNASNone?ïfXÚ6µ?•bO@à?"4äºßwe?•bO@à?í«ˆqm?µÓ©MÖG?·Ê§Jàš?µÓ©MÖG?í'ŒH¼÷?¡‡€ß°Ìˆ?·ósœÞ1I?¡‡€ß°Ìˆ?î±²Xñø?ö[…o' ?®ÔäÜ(®w?ö[…o' ?ëLQ§4_?¿
§Š_Â?Âιc/òƒ?¿
§Š_Â?ØðC`
B?ϒYS®Rä?ã‡ÞOù^ó?ϒYS®Rä?ä_Lœ™[å?¶Úe¸QÑÀ?×AfÆÍH7?¶Úe¸QÑÀ?á'ß7]R?·=ì«î?Ý°A'Dá[?·=ì«î	MIXED4FGL J1612.4+0409¿æ·ÿÈøÜ@Bu"úÖËSÀ;Ÿ$`2À<±ÑtÒ9ô@ò§´i??ü¼˜6Ã
¬?϶ÊÂ["¶?Ø×@	,LÄÔ°Ç@+e¢F;?ïæ'j(¿âûjÚim'¿Ü&ŠwÔx¿ÑgïØÓÁ¿í
â18¿ïÿ›÷Aë]UNASNone?ïÏ轐'*?wp"cV?x¡OÃ
?wp"cV?ﺌ,bx_?‰qà¶òA'?\ôãšVF?‰qà¶òA'?î.L{Ê?š%•O'Ö&?­;>ü\`?š%•O'Ö&?ï32(`
F?|÷ùփ?™™ºü•½A?|÷ùփ?ïÃãXǯ?Èß,uÔÃ?~SÛï\s?Èß,uÔÃ?îM¾>?´­(d§h?¨Ό$?´­(d§h?í
è¼J&?©NúŽ7?·"¸ÓÔP?©NúŽ7?íŸZèr´?£P¼áìEm?·S'œ_?£P¼áìEmAGN4FGL J1612.4-4419¿îzŒåx_@MhÍJ¡À9êIHHn.À;7oE298@×ÆÎ0$5@üa'?ÕГÁ=w…?î÷‡ Q»@ً÷ðg?ü›è~Y!¿ïø罓ô¿?ïï"Áhj£¿ë/¿5_ˆ¿æúÖ?½/K¿Üõ™Ÿ£ÉÉ¿ëþ!²WVUNASNone?îí½ÙÐýo?³¹+&Á­?¡$"bð)?³¹+&Á­?׫~3Æ?Ò²·Ð'R?ä*@æzý?Ò²·Ð'R?êÈ>HBÂ{?ª$ˆ]w£|?ÄßÞôö?ª$ˆ]w£|?ȧ³5ªi?¼pvÆÂ?éÖ2•\&?¼pvÆÂ?æÖè.¨	?Ñ,6¾û?ÓâR/¢¯î?Ñ,6¾û?¯0=}—Ž?À4i~è?îü'áÎð?À4i~è?âñ%µØOÉ?¹î@Ý7J'?Ú´"O`n?¹î@Ý7J'?_gv}~²?qÌ¢–Q•f?ïðLDëÜ ?qÌ¢–Q•fMIXED4FGL J1613.0-5102?Ý0þ# ²×?½ò6=Ô¢À7Ù¯ÅU	GÀ9Š¦V@~u@ªŠÀbÜ@r.þñG?¾Ì¡Ù¯l?Õb'|ñ˜3@¯ªŠ'¥a@ ¨²fD¿Ò[—?ø¡¿âG¦Ý¤áK¿à—à?ñ2¿è›U%ÌBc¿ìQ'[¶¿ïþ£^"_ôUNASNone?»÷Hó±5?ÛüPÚ?ìÖá‰Ù?ÛüPÚ?Ä×0üª¾Ž?À[âø!?êÊ3ÀÕP]?À[âø!?ÅÉ8ï6Ñ?®"d2—rq?ꍱù"2L?®"d2—rq?Ò³žá_´y?¹‹±ø«ºé?æ¦0P%Ã?¹‹±ø«ºé?Š°`óoTË?¦Ã¶Ó°#›?ï•>|M¿?¦Ã¶Ó°#›?Š7­…"­ï?ûõݦ߉?ï—!J0-x?ûõݦ߉?¸"`i/S?§DßÀàÔm?ìísóµe?§DßÀàÔm?s«ÙwU?pcöª'Ô=?ïبM;?pcöª'Ô=PSR4FGL J1613.1-3840?×íAG¯'\@"$§Ös>¼À:°ðs›OÀ<
N‰Ðκ@ ø*$Á«\?óDJè[žŒ?áŽ-àc­?àÚ;ëh™G?þ1ßÈR@Ž¢ÛÔÊ?çZ,Ñð"<?ïxe!Aï¿ës…hŠ-?²(þ¦ä†¿Þ……zþ£ß¿å̂$2pUNASNone?ïìÅW¯á§?t=ÝA[w?c:¨GßI?t=ÝA[w?ï½ØC´›å?Œ/(ò©?€‰ïpÌ?Œ/(ò©?ï9bÅ¥™¶?'+mð]™?˜Ó§I"ûN?'+mð]™?ïç]I‡2?S‹GÔý^??h¢¶™É±
?S‹GÔý^??ïϔÍ×ä®?À&'=õ?x5™.*°ç?À&'=õ?î^^¸¥¬?¹"©:†œ?¯š*"F?¹"©:†œ?îW
y:? s¶¼,P?ª‡$÷`h? s¶¼,P?ïÄDù'?t"*4†?}ñ]"? œ?t"*4†AGN4FGL J1615.3-1512?ëK¨R¢˜@8è"Ýz™úÀ:ŠŽ]%uÀ</j£	@­w'ÃiL?þ:‹KøüÖ?Òf';‡?Öó{!ßMÙ@f"f\Uk?ÿáJø÷£?æ'$óÅ¿æ´2ÝeK?çè?º*2Ù¿å6<!ÄJó¿âõ@S­&>¿ïþ¿UØUNASNone?ïô'aÿ]?Vzµ
åå?W±<Ûv‡?Vzµ
åå?ï<»aŒÚ;?¡Ìx0?˜h"̬ê¥?¡Ìx0?ïñސTÞ?!7£©i¦?œÄ,=–Q?!7£©i¦?îÛÎüì"?ˆ_y"$?¢C5'Bæ?ˆ_y"$?ïíÁþ"ìO?kkF°«–?b>ì¨P?kkF°«–?ìËÙ8\,?Áç<Ò:Â@?¹¡7¦=¢?Áç<Ò:Â@?탔ñ$%?¤VUL7¼?³ãXu$(Û?¤VUL7¼?ëá³1MÞc?¯îü9±X{?Ày3:Ȇu?¯îü9±X{AGN4FGL J1615.5-5434¿ïÄÝ)¼<À¦°'ª¸À9á÷¯îpÀ;Fʨ/^'@Êx‰©@'ì®êc·?Çîüâê?ºd Ïª?ðxºvˆóY?õaDì³r?G)Š=¿éG1b"´á¿ã
'ž*x¿èVlˆ¿VÿáÁ*l»>¿ç+YnLUNASNone?ïõãœr?N…9
e)?T8Æ»¨Ç'?N…9
e)?î拽°G?ª¸E´Â?¡ŸçCI—?ª¸E´Â?ÐôÇ	?‡Jt¤Øí?»ï¼?‡Jt¤Øí?îïî˂Ób?"²ÊÜÌc	?¡LLØ?"²ÊÜÌc	?ïÆÄ4¢Éï?v±Æ…æ¬m?|åºù s?v±Æ…æ¬m?èDOS‹~Š?ÍLŒ?éÏè?Îî±ÒØ?ÍLŒ?éÏè?îtl¢PÞ{?žX×'[É?¨¹5Ø^cS?žX×'[É?åw®—yü?»q"àˆI?Õ¢ÑÜ?»q"àˆIAGN4FGL J1615.9-4322¿Â]VG_e@N0DkjÀ:"A±{7¯À;jÃwï%@ÀØ#B$h@8Omü]?ûéM¼KuI?εN+>?úzDºD4@ÜCR:4"?ïb<jêY¦¿ß	?"OZ†¿ë'ñ¡îQØ¿æn~ãµÇ¿Ø°†zØä2¿êƒËf›?ŒUNASNone?î¢Q÷Í	;?»õD |ˆ?¥Úà†ŸG?»õD |ˆ?ï`0ǞÉ?¡Mü:¸2˜?"ùç^Î?¡Mü:¸2˜?íAó¥~ª*?©]fDyùã?µðbÑäí3?©]fDyùã?ïã«öj?a¹Ážm®L?lTê0?a¹Ážm®L?ëAhD"`Å?ÆCÉ|úì4?Âú^íî|í?ÆCÉ|úì4?ë\ú"Ö?Ç	6d ?Ã¬¦?Ç	6d ?ék˜u4èó?³`ê²ñt?ÊQž+,\2?³`ê²ñt?ízßäM?°àzaâ?´)h°ª?°àzaâAGN4FGL J1616.6-5341¿ê@É)1Û"À[!f'À9]ħd]À;Ùô¦/ª@@§.­'@›Ç »aj?À7™NÆ?ïLùx&'K@!Í¥¹bŒ½@Ô+Ž#CÒ?ïäiÁºŸú¿Ýƒÿ°É¿½¼dãoü¿èŽ?{¿î(ÀþãJh¿ïÿUJÃUNASNone3FGL J1616.8-5343?`å£"Nrv?U£œû{?ïï\¢˜F?U£œû{?µKHßGÎ?±BÒÀ7¶?íV–ãíá×?±BÒÀ7¶?±æñEó?Ÿh¾â'?íßc"GÁ?Ÿh¾â'?'†ÑgԌ?kNȗãPè?ïµäº™g?kNȗãPè?…Þ ÅîóN?¹ ¶¡̼?洞|£Œ?¹ ¶¡̼?…9NaT1D?‡×ãH'ª?ï«ƈm«?‡×ãH'ª?&¿Û˜Y¸?€ÉE93=?ï~ÊZ6ò?€ÉE93=?'¶NŽŸ¤?)¨é ,?ïþ"žq?)¨é ,PSR4FGL J1616.6-5009?ïêÃQgÀr?×ٜSˆ=QÀ8LÀ½ÊÑJÀ9ÍLê"]ð@ À‹–!@ë|þX`?ÉtAEo Í?á3Ï@ŠÎ-±ê?ò!#"'Ä?ËXòŠv'¿Ùµl]÷,¿äM: ºË¿ìZŸ2ਿíTi¿n¿ç˜Þˆ¶óUNASNone?Ö"•ŠÚþ®?Óòa®"K?äîµ:'€©?Óòa®"K?»e`–‡?¶c­ø–í?ì"Sý-<Ï?¶c­ø–í?ÓdZÝò%?µ,,Z†F?æMґøî?µ,,Z†F?©Pçf;?‡vÈs'î?ïêµk^?‡vÈs'î?Ú¤üˆ@º?Ù[T,°•½?⭁»ßó#?Ù[T,°•½?†mo·Kp?‹žÆªö5?壘J
)?‹žÆªö5?²ìûË7ØQ?§K!I´¦?í¢`†Â@F?§K!I´¦?*Gš#(«?"0
CÀMº?ïþ[†t´ï?"0
CÀMºPSR4FGL J1617.8-4418¿àûÌÉ¿¯@­ò>v]TÀ9é:G#«À;všÛ¸ù@9(_D´@=˜¿p?×è^"Ë?ïþ©SK¯@ÿSŸºE@£ñ~Ý֊?ÜÄF€íÑ)¿ÔùQ$µÁî¿êQˆÞ¶YC¿ïþð g?ï(J®kc¿ïý¬2ùQUNASNone?㙯'Üš?Ñ qac"œ?ØÌ ÜGØË?Ñ qac"œ?è«8
ɨ?ÐO4üø9?ÏÑSÈÙ^?ÐO4üø9?çŸ(ª¡²J?±¤\wAƒm?ÐÁ®ª¼›k?±¤\wAƒm?ïyîŽ=šë?Žew³RÄ?Â.;¼>–?Žew³RÄ?Ò(~–Uc×?ÎÐ!×úº?æëÀ´ÕN?ÎÐ!×úº?¾H`Û¦É?ÊFßö¨Æç?ì6óä‹&Ý?ÊFßö¨Æç?Ý·aous?ÀB†Uw´J?áw$OHEG?ÀB†Uw´J?áÌM$öÚ?ÒÌÇw?Ügáe¶K?ÒÌÇwMIXED4FGL J1618.0-5119?çÞڇËf¿ä3™Š€!#À8aOZ±&~À:`ÇÀôQ@ ®¤¸Üó@¢ñÄÓÚ?Ä©ò­1&?¹UJ4VžÈ?ü­ÚB×@›cÇЎ£?êÐxR÷ô™?èD
úú?Èrè•U<H¿åe»¡k5¿éDù>oÒK¿ØøÒy´÷ÄUNASNone?æځÐ>
A?Ѧ
sÔìŠ?ÒJü_ƒë?Ѧ
sÔìŠ?înÖRª?¸+sR0o!?¯"R£_?¸+sR0o!?àrî
c?ºáÆP~??ß#ÿÛå;?ºáÆP~??ëégv Š?¬Í$ÌÃ1?ÀZb%}׶?¬Í$ÌÃ1?ÖaÔ§Ïo?Ó^_—üFÉ?äϬ1H?Ó^_—üFÉ?êƒ?Ë¥÷?Ì.-Î"?ÅóÑiÈ#?Ì.-Î"?àrŸs/?ÂKWÏJ'?ßÁË¡ð?ÂKWÏJ'?Þ±áR¯i?á╃VÙ?à§~Ö¨K?á╃VÙMIXED4FGL J1618.3-4537¿ï«¨¥ƒ»@RÍÀÓgÀ9Úl <K
À:#ÍbôÁÞ@渭Ûð×@ݺZÚA@m">5ŵ?âm-êñÑ@»†Eÿ¾'@¾n¢Ÿþ?à‹)ßwtV?Ú÷;ÀöTÛ¿ê±­ÿ"Z¿ìaÄ@6Põ¿Ñ/AÁÁUö¿à3½Ò^FUNASNone?åáZ,â?ÕN<îЈ?Ô=ýKŦ=?ÕN<îЈ?ìëz¶Ä;?™ÑÚ ƒ?¸¤*I<?™ÑÚ ƒ?æ2XÅòp©?²®Ÿ03Â?ӛNt®?²®Ÿ03Â?ïÓ1ÜÊF?zfÿžÊEµ?vg1"Èèù?zfÿžÊEµ?å…Ly;'b?Ñ/yŠ…†?Ôõg
ˆÝ<?Ñ/yŠ…†?ޞ[ÖüŒ¿?Õ~qDƒÆ?à°Ò¹ ?Õ~qDƒÆ?ænQ†V?³¸r݌}?ÒÅ#\óÃS?³¸r݌}?êL-ü£»B?Æ[\ûŒ0ƒ?ÆÏH
qù?Æ[\ûŒ0ƒMIXED4FGL J1619.3-5047?ï[±V7
¿Ø¸"*}ØÀ8¡.¢ªºÀ:¸ÒD@ƒ8XŒ@x@@aïß?Ë"">Ä6?Û²Çë¼|@®ˆã—?öþJ«ŸÖu?ÖîøüU¦{¿ålÿ!³®ï¿ÜkñUBQ´¿ç…`'¿í«a­šž¿ïrBþx%UNASNone2FGL J1619.7-5040c?мæi›?ÐýÊñ€`?çþz!ŒË3?ÐýÊñ€`?ýƒÔE½?½µ³ß»?ëŸ?Jî'?½µ³ß»?ÑĺiÈƃ?µ NÃl?ç¢Ëœ¿?µ NÃl?½áÌ8RVå?¤GmàÈg?ìCÆxõµ#?¤GmàÈg?©±º^ÌnL?¸›«c7á,?îdäZ ÷‹?¸›«c7á,?Žg¸(®}Š?"xêCøt¾?ï†a¡þ9?"xêCøt¾?°°HnÅ	Ô?¢-–þV9?íéöòBÛ¥?¢-–þV9?_¹P%¬Â?SgaÍ$i?ïð£"q?SgaÍ$iPSR4FGL J1619.4-5106c?í:ôû•A¿ã°™?׆dÀ8=³/lÕÀ9×Ô)¸`.@!GÁntÒ»@'PǙ?Ñ
\^ûŽ?À½y]9!@^aµ&¾?ý|V[?ïÿúŒ"¸'¿ãP'7§¿ê"qh"¿ådÀÉß2¿åҗ¢¡§¿ç®ÿ\lUNASNone?åÓ»"k?ÑìgxEr6?ÔX‰ÉÂ×+?ÑìgxEr6?åÎFS™?ЊNŸÂŸð?ÔcásXÎ?ЊNŸÂŸð?ݛŒ.î?»b°Ï@D"?á29ùÿh‰?»b°Ï@D"?æqéô?¸¬w¸`h§?ÓçÛ,Å?¸¬w¸`h§?çÖ¨Àurë?ÎÍM4U?ÐR®*?ÎÍM4U?ж@Üò'b?Ñ[ÇT³G?ç¤ß'†¶Ï?Ñ[ÇT³G?ÝÙÄîmA³?Àê8",XŠ?áˆÉ_&?Àê8",XŠ?´¡âa‹?¢?¬f;ÑÅã'?íkô'Ì?¬f;ÑÅã'$MIXED4FGL J1619.5-5014c?ïn±Stœ4¿"ˆ&ÌêÌÀ8ȽÇvK·À9»òt&BŠ@ÚhŸ{°Ð@cnda©h?ʺðViÄ?И¹à6*@
Þ ²'/@%'~È2¿ïH¤´Îí?î<|½ÀÀO¿ØbO §)û¿ä†ÞvB||¿ê™XÌIð¿çï7@-ÌUNASNone3FGL J1619.0-5014c?äM[ÝSõ?ÒÀr;[Ë®?×eHEáX?ÒÀr;[Ë®?é$Ýb¤Ã?ÈU™ÀíÛ?˟lŠulò?ÈU™ÀíÛ?ÝÌû¬ðI»?¶(1®ö9?á')‡Û#?¶(1®ö9?ìÃ¦C²C?§¨Ú\àß?»âÍâmë?§¨Ú\àß?ß{F7Fé?ÓîÜÅN?àB\ä\‹q?ÓîÜÅN?ÖÝςÎjË?ѶJµø?ä'>˜Êš?ѶJµø?Ñ.‹~Mã¹?»g–€ú*?çhº@Ù$?»g–€ú*?ÑÓ—aÂ#?ÁaÒCæ?çs´Oî?ÁaÒCæ4MIXED4FGL J1620.5-5729?¹\žÈÞNÀAÄÆnÀ9ßÊKM
À;‰%Þ¶Ú@
œß^@†{¯£Ç?ÈP‰°B}?Ægv[Ñâá?ÿòŸ	E# ?ÿUûƒ¯?ïˆ&_e@L¿Ô
£\ú¿æ†Ž¾`¿è"Ø¿Ÿ<Ç¿éâ<›<¿ïþØ
bUNASNone?ïÎùe?	?wpÈ4w®ö?xƒMP?wpÈ4w®ö?îØ؈º»?¥šæ3›Ðæ?¢rwt^TR?¥šæ3›Ðæ?ï)PÇKa0?}(%·??šÕç*ßõ?}(%·??î°´©H÷?ƒ¡ð'—ö?¤ôµlZ‡?ƒ¡ð'—ö?퀛•PÎ?®Ðw†p?³û'1`Œ?®Ðw†p?èB2|Kwo?ɎÜå|N¹?Î÷6Ò"D?ɎÜå|N¹?çÏËPºœb?¶š4¨«'?Ð`i^ŠÇ;?¶š4¨«'?å2¼DÇä?²°Ï"s9?՛î‡vp9?²°Ï"s9AGN4FGL J1620.8-4958c?ëzî­¿Á?k'Úæ@À8s¼W3Ã|À9¤2ðîE@ÁÔKòç@Gòš¼¯H?Å2"{€ê?Ѫ¿±±=@€Âa8ÿü?ÿÕ©$|>¿î/§íå?ïoÑÿ¼Ž;¿â=à‹F¿ç˜§Å¬G¿ê–±‡Ìè¿èÈÔð‡½UNASNone?ÙDˆ£°§?ӄèrÍÜ?ãu]»®'¬?ӄèrÍÜ?ÕUÎχ?ËÜÂ
V)Ø?åvÕ˜½?ËÜÂ
V)Ø?Ör–‡Z?´Ÿ¨íÔ?äôF¿4¼S?´Ÿ¨íÔ?á[†nÍÙ?¼-‡õ¢?ÝHó"eÊN?¼-‡õ¢?È	•nÖfB?ÓZÿ´šj¿?éýš¤Jfo?ÓZÿ´šj¿? #BÐ45g?ªÔ—£H©?îýËÒü¼ª?ªÔ—£H©?µ~\AÏm?£–'ªÇQS?íP4}áb?£–'ªÇQS?Õ9´ªâ¯?–Ó,›'›?ïV2Lê{?–Ó,›'›0MIXED4FGL J1620.8-5035c?ïÒæ¾Eõ¿Ú¦lü,¶ÂÀ8A˜iòÀ9Ð1T5â:@!
"é3_Ô@¥ŒÄŸâ?É+å¶þ"?¾bcL€Œ,@Œ$›À»G@¨³Åê°c?嘱…K.?ÏÌ
…&¿æë%(®u¿æÆÕ½â¿æ5þßÄv<¿æU‡Ô>UNASNone?æ9û#wSt?Ñ¡ì[À?ӌ	¹Y?Ñ¡ì[À?éo~VáÓ?Êóéïûو?ËÎB¤xµ?Êóéïûو?ÝT¬]&Þ?»8¢³É›•?áUû©Ñl'?»8¢³É›•?é)ïpCh?²Y\ÿ]¹?ÊXB>òb?²Y\ÿ]¹?â–Ìö›ÛÇ?ӭȳ–"Ÿ?ÚÒfÈHr?ӭȳ–"Ÿ?Ü?‡Oj!?Ô?µ˜äÏ?áàq<XJð?Ô?µ˜äÏ?ÙH`ŽW"?ÄY蚙Úî?ã|ÛϸÔ6?ÄY蚙Úî?Åìý€-?·¼#²¤¼ê?êºÄÀŸþõ?·¼#²¤¼ê4MIXED4FGL J1620.9+4852?éòŽ¶š9@F>dÜY2À;'òvªHÀ<÷#ý5Je@4½ú¢É?ÿ‡ÝDUG?Ñ+ä<U?Ç#õ}›?ôý›yÙ
@·]`XZ_?ïÿþÞ÷¿í­x©_	{¿É£èg‡ù‰¿Þï0ês¿î
▸"?ØËWí»°UNASNone?ïêúlÃ!Ó?vãf[o?e'ø%ý&?vãf[o?ïðJéÛc?`píˆ}–?_j,ƒ"‹I?`píˆ}–?ï}qŒN[?"ÔçYˆ5?QÎ{cþ¡?"ÔçYˆ5?ïÓ¾¨"*¼?[ª?RR®?v «É(qÉ?[ª?RR®?ïðč°y§?`
IršfE?^väôCÙ?`
IršfE?ïÅÊ	gÍ?4v³rT"?}p›
*¤?4v³rT"?îñ®Ñí¦•?–Ðò¡G¸Ñ? åݵúº?–Ðò¡G¸Ñ?ïH +L=?'–7[F?–ý[ñÿrx?'–7[FAGN4FGL J1621.0-2625?ÖÞ]C/@0sï¿@PÀ9ÆÕ©²ìÀ;t	§H®Å@»¿Nßáý@÷d[ËÙ?̈́Q2øzÑ?Ø"@Îé@‹6¿y@*ö'©¿ïê~ŸBP?ïÁ0αÿ¿éåϽ—ûŠ¿ç¸ˆû¼¤¿ï»Þ§j¾¿ïÿö$´ë/UNASNone?ï²'˜ÿ?…ÉRôãz
?ƒ|vN¸=?…ÉRôãz
?îR%Œ£ß?®óyé2ۋ?ªÖ-¥}ô?®óyé2ۋ?íüP·Â=?¡Ë6`"û?·€{ù¼?¡Ë6`"û?îàðìDið?…'Ã4?¡ðñ:"?…'Ã4?í²Í{ã&?¶å-"§ë?²i""T?¶å-"§ë?æ=fi…C?Ð}¿AHö?Ӆ3,õxà?Ð}¿AHö?ãbÿۆ½¹?º.²½Nw?Ù:Hò"?º.²½Nw?ç9ÂïS_?¹g_aïœ?ÑñŒz!YA?¹g_aïœAGN4FGL J1621.4-4511¿å4kžxjd@
ª}>ïÿØÀ9ºÜ€žöÑÀ;n4Ïë@ï²>+3à@lX–š?Ô§]7¼?ÔïŠ|p>@O@4£v@+
y*¹<¿çtí²öaò?ïҀÖT5¿æÔÒ$ú¿â
Ÿû³j%¿ïÿyÈBúQ?î"ò¨ÿh+UNASNone?îK÷C:_?²ñ–=–$?«Oð‰8¥?²ñ–=–$?í$ñf²O?·åxç³³?¶ØtφŠ?·åxç³³?êv3ˆ˜•c?®j®#Þ9X?Æ'1ݝªu?®j®#Þ9X?îÀâNFèz?Ã‡Z¦	'?£ñÛµ'\?Ã‡Z¦	'?åú]'xQ?É»‰K¡FÀ?ÔDû]õ?É»‰K¡FÀ?Ù0{ÞGÉm?Ò}i&#?ãgÂÜI?Ò}i&#?ÜÎ
*Œ¿?½P
Õ$p?á˜ú깿 ?½P
Õ$p?áèÐKåå*?À¿#dn•?Ü._h45«?À¿#dn•MIXED4FGL J1621.9+6706?ßP×MÚ(€@C‡á2µ^òÀ;.÷<À<§]k"@;rW3C@§ÒŸt¤î?¿ìðXõ¿ºEik©q?ðÌgL?s³?÷,¨‡ª?ï͎É[ÿ¿êÙ"±ð*¿èÌÝÓ/g¿à‹ èBt¿ïüQ¿æ4}¿î¬é!í¸UNASNone?ïïR0¬ù¦?j/4ˌ¤t?`­ÏzáÑv?j/4ˌ¤t?ïC:ߜU?§2®uk3?Ÿw˜ªë­a?§2®uk3?T	}¾?‰Ë–Œ‹ùz?ŸêöÁXt?‰Ë–Œ‹ùz?îÃR]q?Œâǜ'í?£ÊÚ._8ö?Œâǜ'í?ïÜÌy1D?tÜ×	#X·?q™þ-iÝü?tÜ×	#X·?èéð/c¬?Ë^t#,CÅ?ϨX?BqP?Ë^t#,CÅ?ï}'Œ·³á?Ž"²~XOÁ?O®e™çç?Ž"²~XOÁ?ä§ü.ò=?»|K¦U??Ö°£Ò…?»|K¦U?AGN4FGL J1622.0-5157c?çáë¾nT¿øÓíçÐÀ9mbÙéìÀ:´&Nyá@䉱ïý@ã¬BÊ?ąÿb$?Á	WC¡ë?ýö5{âÏn?ùDÔ:ªJí¿åvw@(d"?ïâÜ~E«0¿å`i,"A¿åFÁ+Xô¿ìÞJZƒÚ¿½Ãø<èÎUNASNone?ï3YØÅ»?¡Kª
Jh?™"Ý!w¬±?¡Kª
Jh?ëÒ}k:¶Š?¾:lÆ Ÿ?À¶
S%×?¾:lÆ Ÿ?é§ÉùÍ{?±sâŒzíÊ?ÉcØÊ?±sâŒzíÊ?ë·mrc?¥ß‹*EB?Á#'J6sÉ?¥ß‹*EB?ãÝƼ‰Ö?̓qˆÆm?ÙÌDr†ìT?̓qˆÆm?ݲjG?ӑΚF,?á&ôÊÜv}?ӑΚF,?äȀbn'¸?¹{'-F~!?Önÿ;"ڏ?¹{'-F~!?ÑÀ¦ûÏ;3?¼(¦Ÿ3?ç¬'bf?¼(¦Ÿ3 MIXED4FGL J1622.2-7202¿íÀ':+ŸìÀ/þKZÀ:}"ç¨ñ%À<|ɳ<ØÎ@¹âÖysß@$  0÷ð?ÂZŸÞ­?ÕðÖâz^@[è¡>©‰?ùzÛž?ïÿÝƒ(i¿ÝæüÅW8¿Ø¾\ý1§¿ä‡(mÀοì¾}ÖÅt¿ïÿ¤?åÉUNASNone?ØbSd߆@?Ç<]ö¢«ˆ?ãÎÖM<à?Ç<]ö¢«ˆ?ånA…±Z?ÇA¤$·ðG?Õ#Õ|ôK?ÇA¤$·ðG?ã9†ãÑt?¶Xá¿3mQ?ٌò9Ì]?¶Xá¿3mQ?è5gŽ&?¦uCù?Ï)¾aÇg«?¦uCù?Äqˆ"Æ ?¾½å'•
?êã¸]÷Nx?¾½å'•
?Ƥ À-ÆÑ?Æ~6šæ ?êV÷ÏôŽL?Æ~6šæ ?Ãc½ÙX»?²Lð˜øœ?ë9物Ñ?²Lð˜øœ?˓3Âö-?¬ÊÔ«ç›?é3'u?¬ÊÔ«ç›MIXED4FGL J1622.5-4726¿ê'mí™K?ùý ½é¨À9V3é;˜À:²xþŸ3@®hÌr3ú@tÝdʄô?Èë¨Z&½?Ïl¡ÿCÂx@Ê:#}?ÿx-
TQf?î˜ÓÁ2º½¿à´Ҟå¿ç€ÔÜeÇ¿è¡Ý4ùÝ¿éTô¹zàq¿ï¾á77¥UNASNone?íI‰˜é?·òª'jt^?µ³·bciµ?·òª'jt^?è¤Ðü©«­?ÃMÓX¾C?Íl¼
YQL?ÃMÓX¾C?é¼°ØOŒÛ?²Oõ[²?É
<žÁ̔?²Oõ[²?ë)óËH?¢o`ʕò?ÃX3»ÌÒà?¢o`ʕò?ܤµb^*>?Ê`l¾ç~K?á­¥NÐêá?Ê`l¾ç~K?ƒtÕG£5?ÇxO`ÕÀ?ê[bÊ®3?ÇxO`ÕÀ?ÖkËL'u€?»>­¶mK?äÊY·E@?»>­¶mK?ÍÂí6?³¾¹ä'¼?蹺|ÏD²?³¾¹ä'¼	MIXED4FGL J1622.7-4934c?àZk›"€?·†×J)CñÀ7Ò'D:ÂÀ9bÙéëÂ@J2Œðø@‹$ÜX[?Á5šìð?Ô¥lÞ@9É oâ?üç`¬"{¿áø"0¤º?î[R¡ƒâ¿àZþ¾·`T¿è+Öþ)E¿îW}à€ˆÑ¿ïýÜÚa
UNASNone?¦¬º)N[l?º:,yÄx?î•4]][Ù?º:,yÄx?¼ß×"ˆz?µF\¥Ut?ìd®îQ?µF\¥Ut?Ä!Ï
-š?°€gMfò?ê÷¼Ì=t™?°€gMfò?­Ó¿‹>ä¢?˜6#ݽ¦b?î"Ä"Öf?˜6#ݽ¦b?°üUº<iw?Ë;°€÷óR?íàuHy?Ë;°€÷óR?ˆWöÁO܅?Ž–î®ã™?$ßC®?Ž–î®ã™?'˜xâ]æb?‡àÁæ—?ïk<9L?‡àÁæ—?FD,Ú#"??0…:ù©Õ?ïúnõ<hÍ??0…:ù©Õ0PSR4FGL J1623.0-4624¿ïŠ˜çå¾@Fb\ìj!À9e3ÔBâÔÀ:àŒ]"Y@†zº±AV@ÛµûÏï—?Æë΅3±?®[!3‰ù?íºüÀ°^Ø?ù>&×/QQ?ïº8À»Çl¿ç*.<Sme¿êú©u°¿å>`"†É¿ç–&ÇUj¿à0«¼²UNASNone?ïȃ÷î?vÀž½J?{À>r¤0Ð?vÀž½J?î˜<;¼æó?«l| ª	?¦|<@ÁôÔ?«l| ª	?î$ãÍwö?¡JÛ1ɹ?­±Ã'¤¸?¡JÛ1ɹ?îÂÏÏFàË?‰¤-{¡&¥?£Ó	Ú%N?‰¤-{¡&¥?îû²n?­]'‡Á?¯@NɘŽ"?­]'‡Á?æd;zÍ?Ï«ãäý\?Óï7‰àg?Ï«ãäý\?ìþ¸¤™õ?§åkqk'Ä?¸
?bÛ0W?§åkqk'Ä?ä'Ž®¯?»[só[›¡?×±æ⢢?»[só[›¡AGN4FGL J1623.7-2315c¿»³ìT\@2"ëÄØíÀ9»øç
¶À;&ߢ'fŸ@_ºžLè@øb9°û¶?¯1†_Õþ¿XßÜÛO?´ýò^¬³¨?ÿG[iUŠ¿æˆ®Êä?ïüœh€òÚ¿ç%Ž?w4¿élëá:(¿è¢™ó[¬Ï¿Ú‰=UöØUNASNone?ïîJÁeW?kLåC¸§×?aµ?4ï?kLåC¸§×?ï±Y¥;—?'ñڔJJ?ƒ©ºEƒ_?'ñڔJJ?î҂âP 4?•Z~v‰'?¢×Ñ׆`Ã?•Z~v‰'?ïÌ(éiw?d£ð¦ý?yù랉?d£ð¦ý?ï2E&r'?›ö>÷fÈD?™·[0Q9?›ö>÷fÈD?íë7c?¼Ÿ×D
æ?°¦DåÇ¡h?¼Ÿ×D
æ?ëŸŐ¡?«¡æÒÙíw?Á'é½|?«¡æÒÙíw?íõ-îȧ?¢.Öü'b­?°VŠ›1Ç?¢.Öü'b­8AGN4FGL J1623.9-6936?åä/]ÜÀ+í²'¸#ÈÀ:]½‹ç)À<uƒ/ÊÈç@i"¨ò?ÿãf³"@?Âçښ?ܺ?×€
Qh@~3Auì@F-ðS:?íþ'›ýø?ä:ÿ°Nè¿Ý¡ªÌô»¿ßBL`€É>¿î9ÎWçG¢¿ïÿÚ«² ÒUNASNone?é"EËM?Â,1ùĞø?Éï›êèÒÎ?Â,1ùĞø?í*Ð=š•B?µFJ%Z[?¶©~Onð?µFJ%Z[?ãX—ŸÖ?¶93ðuÝø?ÙNÐÁÄT?¶93ðuÝø?í¢Q^B‰?"iúbœ?²íw3­4?"iúbœ?Ùm¾næ?É¡aøK3c?ãI øÈÿ
?É¡aøK3c?ãÅQq?г2Ùu?ØÄu\ÅË?г2Ùu?ÐÉü¢á—?µjsÐØO?ç›ü.5?µjsÐØO?äwp7Ü¡g?µÄ…%aµ?אF½1?µÄ…%aµMIXED4FGL J1624.1-4941c?Ü1	¾º¿Ã½?æõÂåÀ9eôݍqÀ:ß`ݐi@¯ÈV"Õ@Û`
†Ñ?Ò:Ùâ)U?ä_Ä@Œ70@[®¤Ã™G@!­Ý|é?åÁ¡ŸØx¿ê"ɞoc¿Çnיå¿ã؀_5ð}¿ëæÕÂ>ÔQ¿à¯ÖòÀ|\UNASNone2FGL J1624.0-4941c?çxJ8ª¸È?Ë
Þ5¼
Ä?ÑkŽªŽp?Ë
Þ5¼
Ä?財ŒúqB?Ä¿iÞ§&?Í5yÌ:÷?Ä¿iÞ§&?åÁ&&–}ì?´(mlËøj?Ô}³²Ó'?´(mlËøj?èûÀ³Âm?­@y
ô?Ï°ý0öK?­@y
ô?Ïwóä`3¿?Æmaný09?è"çó?Æmaný09?Ê94Z‹Íå?ȉ4É­ªë?éq²é]‡?ȉ4É­ªë?ÕjkaUŽ?ºmµ>†b?å}ÊÊOU9?ºmµ>†b?Ê­r˜¹?±£>ݙb?éT£{Ѹ?±£>ݙb0MIXED4FGL J1624.1-4417?ÐCžã@
—Ne¾¡À:8;fÀ;EÝhüBÜ@äÀ^g@ä…BÊë?˲&˜Æ
?Ø/s?è£B@WÝ¢&e?÷s7µxó1?ïþsè¿ãã'ö»3¿ÛØ´¢¨ñ¿å‡ÐO¹¿íهÆ2~Ø¿ïùñ]¥Í…UNASNone?éI-+Ãc?À?:ŸÛt?ËÎÛKPòr?À?:ŸÛt?×åd¬/¦ê?Ë3¿Žåz]?ä
M©è,‹?Ë3¿Žåz]?é¤OƒÝ?«lÂr—&?ÉnÁð‹ÿä?«lÂr—&?áñ]½lÔâ?²bû(Óÿ?ÜD…&V<?²bû(Óÿ?ÜÐ{}žD?È÷ª*$Z—?á—ÂuA0Þ?È÷ª*$Z—?¡#øѺ&À?®íÃK‹?îíÀrÿÚt?®íÃK‹?ÙÄ|
+kØ?·G5ùÜÜ?ãÁúêJ?·G5ùÜÜ?¨‰®ƒÐHq?"±	UqÕ
?îweÂûy?"±	UqÕ
MIXED4FGL J1624.9-4538¿â­8¡Î@®ò"z–À9½ï}Ѽ÷À;)²ì`@ub
fE@ܝ 6×?Ó¶@ï3?éDGÝå#@LRç-¡#@‹ä<€?ïñ©ûçl‹¿åø‰|ëä¿àø›ó-u¿îh—c^t*¿Þ}z¿ŽËµ¿ïÿí )k3UNASNone?ãó繕Àû?ÍdA*=Ó?Ø0ŒÔ~?ÍdA*=Ó?Þp‹-p&?;@örì?à÷ǺiGí?;@örì?çôÔ¶%@?°æŒ™.y`?ÐV"µ~ý?°æŒ™.y`?æÀ'(˜
ß?³D¯q%~?Ò~Ý®ÏêA?³D¯q%~?Þ
l	h‰?Ð #¦Î5ƒ?àùIûK»??Ð #¦Î5ƒ?¡À;r[Œû?­ÃC:?îãüI@ð?­ÃC:?Û!Nõ?¿¶@ï3?âto|u؅?¿¶@ï3?·†6®€e?²ZW&#øz?í9*1ñƒ?²ZW&#øzMIXED4FGL J1625.3-2338c¿®Ñ;\«"@1š'>[…bÀ9éÊ¥«ÔÀ;Î\ïÅ@
Ù æ@ê¬azŠ?×n†ÆX>…?ãb_p¨à@<÷S½@W?	*K-?ïÿwåëo¿å»Û¾,K
¿ç™ö!ãÕ¿ëõækÚC®¿ïÿÿÊPË?ïü!~|UNASNone1FGL J1623.5-2345c?íÂk¼ð?»¬xeä­¶?±ï¼ Î¤æ?»¬xeä­¶?ç×¹5§gõ?Ê£žô*?ÐP"±0?Ê£žô*?ëpß	ÕÃ?§MðÀW‡?Â<ƒØ«ìò?§MðÀW‡?ìÇ;§À?£/*Ši¼?¹Ç¾"Áþ?£/*Ši¼?êË/–pšG?Ç8qÜf?ÄÓA¦=–ä?Ç8qÜf?Áÿ²Û½‰?Çú<;ðq?ë¸@Iž?Çú<;ðq?à"—"[Â?·ÈHÉÚl?ÞöÐ×H{Å?·ÈHÉÚl?Ì
º…ލ?»z™½ðÉ?èü¿^ˆ]?»z™½ðÉ(MIXED4FGL J1626.0-4917c¿§Y¾{:翶aTâÀ8D*zýÍ À9Úqvdá+@<†¯Üüñ@)Á'°—?Ë;Á·šám?¢*	é¸ÀÑ?æÕÊ@qà@;†rJuD?áXsÉü7ô?¹¸"늿ê恗DU¿ç!Ú{9¿åŠ*@Ejm¿Üëû¼#‡DUNASNone3FGL J1626.2-4911?é0œbvª?Η'¡`k?Ë=Žv$õX?Η'¡`k?ïýýÈ?"wej§Ž†?ˆ¼¸ñø?"wej§Ž†?â—V–9½¼?¸+~$C¥?ÚÑRӌ"ˆ?¸+~$C¥?ïgcîß=µ?}Æâç94R?"'*÷U?}Æâç94R?å´cÑØò—?ÒæÉ<
f?ԗ8\NÑ?ÒæÉ<
f?ílÁG?ÀCÉV˔?´ŸŸ1õÆ?ÀCÉV˔?ä
¨G‡S?¿Wh|¯?×ê¯pñYÊ?¿Wh|¯?ê/¬Ãl?´®H".ÕÝ?ÇALóÆP?´®H".ÕÝ<AGN4FGL J1626.5-4406?äZWÇàª@£&Æ=f"À97RÁmóùÀ:þ›H"@Eªs]@yä"rÁ?ÄÚ^ZÔ6ù?ű9ÉOj@
f H	"@¦+Š¥?ïÁkoº£?îÆ>¾+Ê3¿ä¸R÷ô˜Ä¿âçfá¶hÝ¿ëw¡Aƒ­õ¿Ý+m×sï¼UNASNone3FGL J1626.3-4406?ïÇ÷C ™±?ƒ0Xņ?|^d{?ƒ0Xņ?ï^Põ³BZ?š-ó*?"5áB¸|Ø?š-ó*?î'2C É?Ÿž$5ø?­ŒÛÒñvr?Ÿž$5ø?ï'n[¨G?ƒë®Õ
?›6BÅ?ƒë®Õ
?í+"NšÜ?·6­`"Íÿ?¶¤[egŸ?·6­`"Íÿ?맇rÇë?ÃûÍdæù8?Áaâ4àSà?ÃûÍdæù8?èÁ7§ÙoÀ?´äD0Þ#Ÿ?Ìû!`šA?´äD0Þ#Ÿ?ê0GÒÁGL?³Qy0Ç?Ç>à´úâÏ?³Qy0ÇAGN4FGL J1626.5+6257?ïÿÇ»•²@Dß°Õ À;j‡È¶½—À=
eÀN@ uVÞ^¼?ýƒ_0Ð?É W£Õݘ?°Bq>±—?æ¨B©È¼@}¿AI¿ïÿÈl뻥?ïü¸¹"Š¿ÊÅ¡ŠSÖl¿å
"Þ|L­¿ÂW$T9¿ãkŸ‹K"UNASNone?ïÿvMP¦?8ÏpëKz?6W_"?8ÏpëKz?ïö"§"Ò?UʟófCË?RÖ±bC-0?UʟófCË?ïî@:
p?bÆá&Ô0À?a~Àî*?bÆá&Ô0À?ïüŒÈGNk?&$†Xä?;™¿'>¯J?&$†Xä?ïÿ-³¹Î?ދ%"í»?ZP@i%ô?ދ%"í»?ïÛro3>œ?uB¯¾¦CÎ?rFȂ}õ?uB¯¾¦CÎ?ïäÿíû4ƒ?vÝb/ð¿?ki$à?vÝb/ð¿?ïõâ$¢Ìž?HœE¢Iâ?T;¶€­Sÿ?HœE¢IâAGN4FGL J1626.6-4251?ïþq[Êy@>­\ÄüõÀ9«ã°> ÍÀ;
»y¾1ÿ@ÊÅ&@ù5žG~D?ÍpÔ©e«?ӝÁÓÊm@íÛ¢R¦?ö­3²_
W?ïõ=߉'æ¿äS«Èp¿ææq¹€¿®¿æì´ÿP­—¿îí47³K¿ïÿ¤''UNASNone?éöéKÀ?œ>iœÚ?È'€[žÑ?œ>iœÚ?ÜJÿ6pCN?ÌÄG´åÿ?áڀdÇÞY?ÌÄG´åÿ?êh0R6?¬ž˜ôè{¨?Æ_ÓÃ>·(?¬ž˜ôè{¨?åGîbE?¯KWǘ?Õp#;÷Ûw?¯KWǘ?ã-R¨»ÂÜ?Ê#uîø#p?Ù¥Z®ˆzI?Ê#uîø#p?¥f÷pdl?²õ½Òä	?ˆµ?²õ½Òä	?Ú½2xo ?¹†š¬ß´•?â¡sfÃÈ0?¹†š¬ß´•?±n'
¼—?š"°‹)'–?íÒ/¾šÁ?š"°‹)'–MIXED4FGL J1627.7-5749¿ÕbùõN÷ÀȞºjÊyÀ:%µQàÀ;ï 8"«Ì@|T{,q"@‡ŽºB†?Ų`$'ì.?Ûk_ý–™@èAYB@‰,™»þH?ïJ¶Ýw>ü¿Ò^©Ã(ß¿å"áu¿èì]60¿¿ïýؾ°»¿î·Œ~~
GUNASNone?èÕªÖÐ(C?ŸΠj!?Ì©T¤¿^ò?ŸΠj!?åQn]3?ƟcæŒïñ?Õ]Èý#E™?ƟcæŒïñ?éèB7÷­?®ÉÒÀƒr¤?ËÐ^÷ !L?®ÉÒÀƒr¤?èã­î1Ä?£`žâiþ2?ÌsHG8ñ?£`žâiþ2?Òú7<	ú?Ék&ŽÆ=?æ'äaûü?Ék&ŽÆ=?Àû=cêŸ?őͻgÓ,?ëÁ0§<ÅX?őͻgÓ,?Êvƒ Um?±'ÃŒÖ>p?ébxê¥?±'ÃŒÖ>p?Ãꛅ¾+°?¢¨8Ôîël?ëYu?¢¨8ÔîëlMIXED4FGL J1628.0-4920¿Íè¤ÿ¿Öù¦¸&øÀ9¸<ãÀ;^ݚzj)@b6¬j—?ú{à€Þ·±?ÐÎҀÀÚ¦?ê £ylS@2µÖ\?þÃ]¸Aû¿ïþY#¯?î÷Pß@—Ë?ÒO¥¤ê°¿ä}z´ÒD¿ì"{ýýFg¿ïüÂÉ=ÌUNASNone?ᥐ§ê?̸O‹È9"?Ü´ßÜ°*ç?̸O‹È9"?ã>4ºá©?˪±¾mRX?ك–Š<ü­?˪±¾mRX?ä<ËëÙàå?²ÇÂn´o‡?׆h(L>6?²ÇÂn´o‡?âà=œ1":?´– ášÈ?Ú?"ǜٌ?´– ášÈ?ÁÑRxGåG?½Kþ䪘?닫aî®?½Kþ䪘?Ä£s0½ü¿?Æ&ߎž·?ê×#3ЀÐ?Æ&ߎž·?ÉЁÂã>ÿ?³éÊòµ9?é‹ßG0@?³éÊòµ9?Í1$š?¶&ÒÇãƒó?賿¿6ûÙ?¶&ÒÇãƒóMIXED4FGL J1628.6-4553¿ÖG_}lj ?ÿ<û¹IbJÀ9DçW'Ž
À:ÔL÷)—©@L;´4ç@]X…Ó8?ÊðΉ»U+?Ë0¼
‡ÃX@2/ãšj@÷jt6?ïëÖï썿ä­úNw\¿åé¬Áêp¢¿åË»Š…) ¿îۚû™hò?¿›šOÌñáUNASNone3FGL J1628.4-4546?îƬ¢4ô?±ÆÿîJ;‡?¯•9LLÁ?±ÆÿîJ;‡?î_½¢.á?°x­Øï.œ?¯º!'Žø?°x­Øï.œ?ëX¦¾ßèø?­ù8¡ÃE?e€\ ?­ù8¡ÃE?îJWàø¹÷?V™Œ%	F?«Zì(ݚ?V™Œ%	F?å}J9pJQ?ÇXKT«íž?Õkk^?ÇXKT«íž?áWá('à?ÐE9°zܕ?ÝP=®ûð@?ÐE9°zܕ?áq,ÚöÓ~?¼À~Z?ݦJY?¼À~Z?á–ü/TÆ?¹ üÔMÉ?ÜÒ¡VsÌ?¹ üÔMÉAGN4FGL J1629.3-4822c¿ì*Ȳ®5?ÃÅR.¸ÐÀ8H00IsçÀ9¸ÒãgC@¼HOúê@zÓOž?ÉK⁔ë	?Û	읢'½@Dh¢€Èè@ÞN«´¤7¿Ì°¿%j?îÏ27Š°É¿æ€‡yÜdð¿ëõUҚl¿îpñÚ£O¿ë8¾"UNASNone?áÜ æ©l?Õ*waO??ÜG¾2Þ­(?Õ*waO??Ыó\ó9ã?Çå¢oÔî?çªQ†c?Çå¢oÔî?Ü퇢h?¶TÀ Søõ?á‰<p.øL?¶TÀ Søõ?Ö»K
x?¶6sÿË	¦?ä¢rÚyCõ?¶6sÿË	¦?ÔzÌ©*J?ÖRËÇË9?噫jÚó?ÖRËÇË9?—fGKYu?£±"³Âù?ïDÏ5îà"?£±"³Âù?ÁžëO¨½?°‰Yi?ë˜E>¬Ñ?°‰Yi?"™¡›(Œ|?z%^€¶@;?ﭙyÊWŽ?z%^€¶@;8MIXED4FGL J1630.1-1049?ÌÃäç1@8Ô³_=}9À:™Xù–YÀ<ÈÑÚRÇM@Í_íüG@ÖÝâžÆ)?̳üqU-?ïýò߆õ@ü¥zxl"?þƒÞ©Ä	/¿èQ)/»¯¿ãý›6QË¥?´Gz=ó>¿âWŸ¤¯¿ïÿÌhù¾¿Ú•©Àª€UNASNone3FGL J1630.2-1052?"¡ÂHý?µaÿtJòÆ?ïgò÷/H?µaÿtJòÆ?ȵJúût?ÆÁ\p>?éÒ­AA=ã?ÆÁ\p>?Ðzt{ä
A?°,ÅÌ:q?çÂÅÂ
ù_?°,ÅÌ:q?ªKsêà?'™9êŠâl?î[HÁm{·?'™9êŠâl?·§EaóŠÞ?Í-ÉGÝ?íSêÉô?Í-ÉGÝ?¡'GºŸ?±&§ERY?îî¦ë€…æ?±&§ERY?ÀoâPäì?§˜!N£3ô?ëä9GkÆÅ?§˜!N£3ô?cµ×wQ™p?V›a5s+%?ïìJ(m1‡?V›a5s+%PSR4FGL J1630.1-3546?ê.¿Kz°@!Zt֐›À:o¶Ò"mÀ;Ҋ,l@ .á¿Î@´"¡ºÐK?Ñ¥_ .^?Ø`etÎß@ÿïÕ@Óo¦©?ïýœ
`{¿Þu]¿ä'"Ð=1¿æÐ6y8Ñ¿ïÿÿ)@k*?îÍ<(¥:¸UNASNone?íÐdŒÐ,?º(·Dh1?±|ۘ£—£?º(·Dh1?ê‹÷9ÝÇF?Å[¹Šá×?ÅÐ#ˆâè?Å[¹Šá×?ìÃ[$q'?¢yjtôæË?¹å&Üsïø?¢yjtôæË?î1Ø×5ö ?"v¿.f‹H?¬ârì û?"v¿.f‹H?êñuÒPU"?Å1å[Ë?Ä:(¶¾©°?Å1å[Ë?Æ×=‹s3?ÉfvÝø;?êxJ0#3?ÉfvÝø;?á63Ì=ä?» /µÐ1?Ýý"˜g"7?» /µÐ1?ÚGȊ·˜L?¿>»xLÓÿ?âܺ¤3Ú?¿>»xLÓÿ	MIXED4FGL J1631.7-4826c¿îçn¯hÁh¿ÇYϪ!Ò
À8ª/?ˆ¬À9ö¨y0m†@ )±`_¼(@$,!Æú%?ÒÂI;2[?ț:)Âq@Øm.׃à?ö­Œj1!?âÏàèãƒÈ¿áb×ÖK¿ç…¡êöÙ¿æ/¬*•ÕÀ¿ë¬] l‡¿Þ&«»Z3¨UNASNone3FGL J1632.4-4820?äTÿòÐ(?ÒÃØSàõ?×ÙV_°?ÒÃØSàõ?ãù¹xm`<?Ðk«äc±?Ø%?ˆ?Ðk«äc±?ßutÙLÖ?·‹»Qe¨o?àEE"vٕ?·‹»Qe¨o?åFoX°ú?¶' ;€P÷?Õßs!Nž
?¶' ;€P÷?ÚYÇõ«ÿ?Í­t¯vÈ?âÓ*r?Í­t¯vÈ?¸Ý#)?ÇË®R?ë{\'È·6?ÇË®R?ؓx«%«?¸ÝtÂæE?ã¶C¸*m+?¸ÝtÂæE?­ðÁ1ƒÈ±?¡§×;Ë?î óíþÅ?¡§×;Ë$MIXED4FGL J1631.7-2319c¿ïÆËŪˆ@0²Ž´cI{À9éŽuy)À;_ŸÐê@ͦ;2±@"î¿eÛý?ՔžÝü ?çSfåg1@
ÈÕ[ç‡c?ÿ"˜‹Q­G?ïõûg¿,¿á¿Ú@RÖg¿ë{τ7¿é¡P°¼¿äV 7˜s¿ïõr¾
—BUNASNone2FGL J1632.6-2328c?îÈØqÊ\?ª²c·Væ?£rxíwsF?ª²c·Væ?å-y%ìßÎ?ˋÓú#Ù4?Õ¥
´&@d?ˋÓú#Ù4?ìAb©ÿ~Œ?¥",8µV£?½ôê° ?¥",8µV£?ê±ýrÃ?¨lasª ?Æ;
4ó?¨lasª ?ì±ýˆ×T?¾n
Ø8nd?ºp¹E[?¾n
Ø8nd?¼ö{(♵?År2Wãc?ìa0šã¬É?År2Wãc?ä¸ÌÔsN?·ï¯¤±m?×ȎfWd?·ï¯¤±m?ÆöNY
ê?¸ã#<
?êBli¾=F?¸ã#<
 MIXED4FGL J1631.8+4144¿ïÿÿD¡Î$@EÛLÂPrÀ;zWûi˜JÀ<êîê3@!xáî'Ô?ûg?>Ú0c?Ð$a1s@?µO%,4fd?èË.Ò{bw@PHµP"R?ïö]¿Î¸¿éµyÿ ^°¿çëWÒNí?±·K†;B÷¿åreÊÞ¿¡°lnéÚUNASNone?ïÿ'ên?
þÍv¬S™?¯ÿÐ'?
þÍv¬S™?ïóU•¼Gø?^AÏ)‡±?YTÔ${P¬?^AÏ)‡±?ïù¥Lͅ|?8†i¨š!?IjÌ.â
?8†i¨š!?ïözÁÎRD?:z­NÕn?S
|"Õ×d?:z­NÕn?ïÿŠ+èf0?nOqŠåT?
u¥ÖC?nOqŠåT?ïÑÉYáÙà?}ÊöÝT?wSáC´?}ÊöÝT?ïúh–[?SÔÄçÊÚÒ?G'`žT^ò?SÔÄçÊÚÒ?ïàkà£Ä@?`ß<ÏÝÍ?o"C~B?`ß<ÏÝÍAGN4FGL J1632.5+3839?Þ%¢ô}@Es£]gº#À;k¯{ƒ.À<™·•-#O@–A€h@EbÅÇõÍ?Õò£@ao?ã÷&<ª«:@jÉ¢uá.?ÿÇyü›F˜?ÞýÑÒ¿ê.!EÊål?»!Œ}ãkÜ¿á‰Õx¿ïÿøsCÄ{?ï¢,_Ú[+UNASNone3FGL J1632.8+3838?î
5yAy?¼Äu);§e?¯\¨r["d?¼Äu);§e?í)oöž&?»ðipOk?¶´€J14R?»ðipOk?í!(à·÷?¢ä|[´ö?¶ö¿/°eÇ?¢ä|[´ö?éºdnù2?¬ò$œ­ÐQ?ÉoÎD8?¬ò$œ­ÐQ?쮹ñþµ}?¼ÇùÇ_X3?ºŠ0p
T?¼ÇùÇ_X3?ߟiÜVqk?ÑæªVÞ¼—?à0KÔÇK?ÑæªVÞ¼—?è~Ñ×£•q?¸Øw‰é@?θ¡qª<?¸Øw‰é@?ÖNíäI–!?¾Ð ŠSÆ?ä؉
Û4ï?¾Ð ŠSÆMIXED4FGL J1634.0-4742c¿ëlÂ8²Æ? ?áÜ\WÀ85O«8þNÀ9Õt1*Dw@y(

@Ývh<)|?Æ7d+xª?äÃf,Z@f×})÷J@Œ—Å¡_¿ì.
Ää ÿ¿ËD€7Ñ¿ÖÁ'¡…vL¿çëx‰~™c¿íÍsñidH¿ïÿXÛch…UNASNone2FGL J1634.4-4743c?±È&ñڙ?Á›:-£Q?íÆû!ÒkP?Á›:-£Q?½ôÐjÖ?´ù%cq¦?ìAeò¼å=?´ù%cq¦?ÁéB¹¸óÒ?¬-aô±?녯Q'Ã?¬-aô±?½ðþZcxË?¥û*	<4|?ìAà4³ç?¥û*	<4|?°¯Ú¯=¹­?ÌÍÙÛ0ÆO?íê©ï
{?ÌÍÙÛ0ÆO?‡–nGÚÖ?Ž½y1j?F·Z±?Ž½y1j?—xUê&Ö­?Š 0^m?ïD=PåÃ
?Š 0^m?]-¹(¯'s?SCh'b3>?ïñi#Q‹/?SCh'b3>4PSR4FGL J1634.6-4324?éõ[¯±¼"@ýñ.ð®À9ã'Æf>À;,èI*}@ zËA1xž@ A`ó_ß?ÄkÝþ"…¿"«¦Â?ԕcߣi&@ØÐ,}·f?ïûvΓvj¿ÊQ§g'à¿ãÌxéö©¿âÊÆͯJÜ¿é(€‡yÜe?¾¤nò	UNASNone?ïë(™–z?dB˜_§?d×f~›-Ç?dB˜_§?ïÖUì4Šæ?ƒGXwo ?tÕ	ð¹Lþ?ƒGXwo ?ï†ðüú3…?‰#ïJ/‹ú?ŽCÀÄâºÎ?‰#ïJ/‹ú?ïíežæ‹?MÀ`þ*?bšbµM?MÀ`þ*?ï	̾E[»?¢ó÷6—g?žÆh0uP«?¢ó÷6—g?î'õôÖ?´­:Œù
3?¦à®îéì?´­:Œù
3?í¨5}²ª¯?¤&lU‡ª?²¾Tjªˆ?¤&lU‡ª?ïŒY|j ?}ÓÓ?^H?Œé ó(?}ÓÓ?^HAGN4FGL J1635.3-4159¿ÇÊç移é@
Ϙf"²ÐÀ9Ç DC%ïÀ:þìÁ^ځ@´°z[»¾@‰'¥R5?Õ˲[‹à?êùÄ¢0ìÝ@¸à†½õ?í(iå20?ïþ2Àœ'È¿ÚFUú³dò¿ì†úÆ[¯¿åÄd]øƒµ¿ïþÒn¥Ð?ŒÑt§FÖSUNASNone?æ¦ÊÃ÷ÕÔ?Ñ;9¥¾?Ò²jxTX?Ñ;9¥¾?ÎÛÍÐeß?ʬÚô?èI¹Kæˆ?ʬÚô?è*ý¯˜´?¯ÕÁ…Ij'?Ï»T	A.?¯ÕÁ…Ij'?ėFÎEÄ?¨ÖðûËÕæ?êÚ.Ln˜?¨ÖðûËÕæ?ãm£ä÷?Ôñ皐?Ù$¸6ßÑ?Ôñ皐?"¼¢è_ÀÔ?¤FOp…Ã?ïZè†:?¤FOp…Ã?Ü

oð?¶]AŸh®?áú|zúÈ?¶]AŸh®?h±ý«¡`?['æš$@?ïçåMæ×?['æš$@MIXED4FGL J1635.3+4258?¸ ~—ãö…@E;Ÿ<pÊÀ;VzKöx˜À=WÃ5tV@©Iu¿Ê±?ý1ʘ?&†?Ñ:"Yd?Þ²¾äV×'@©äðl@
¨ˆ±>üÀ?ï 1-Ÿu|¿Ðl¸þæ¿Ô[ÉàhÚ¿ÞaŽºú½¿ïÿÒ³–šâ?ɀ:MèUNASNone3FGL J1635.3+4257?ïñÑ(§*?^}¶ӊW?\]®L%<æ?^}¶ӊW?ïàÀCÉл?s L«q3Ò?o?¼6/Dš?s L«q3Ò?îVÉMŸ?—¼µð•¾i?ª"nLÝÕé?—¼µð•¾i?ï–@¼më?o1"bþ?ŠoþWý-?o1"bþ?ïÖÿEšéÑ?sŸ~AmÃ[?t€]S‡Ws?sŸ~AmÃ[?ïmÔ¿èìF?¢š($2ê?'EgÿrÛM?¢š($2ê?ë81ÛLõÛ?±¤Dº¼?Ã8'Ì(–?±¤Dº¼?îké+8y)?•0qK—?©AmJÀŸk?•0qK—AGN4FGL J1635.4-3249¿æ"zB]¿ñ@#±vû	 À9ç$Ã-èÀ;²F;…è@+hÌÅ@è¡ß¹8›?²¸yƒ¤?Îɹ‡uª§@§æ;2Ûõ@ür׸ä?ïÿÆ>"8¬?±é""xi¿åHpSO2¿æބ 
Q!¿éMd6á=¿ïüNÀ,€gUNASNone?î²»©ŽÚ?±Ã#ùhèö?¯DÔC¯D`?±Ã#ùhèö?ê"ëÑ0
?ÀÇ·N¶Fy?ÇtP»?—×?ÀÇ·N¶Fy?íØ•ô§? y¬:òI?±?ÓO~à‰? y¬:òI?í/n_%¡È?"'	A.?¶"‰F?"'	A.?ä*S÷+£¥?ʘ¿'Z=Â?׫X¨¸µ?ʘ¿'Z=Â?Îqý`	øI?É5³5wE?èc€§ýî?É5³5wE?Þ
¤È½?»{ÑG/êS?àüy-›ø!?»{ÑG/êS?Û+qrÞïº?´ñEÄXª©?âjGFˆ#?´ñEÄXª©MIXED4FGL J1636.9-4710c¿ÓTÁðyÙ? š&	ÔëÀ7˜ÜïY¿À9IeVÏ@6ë¤~O@‹jËG?ÀƇ8n—?ϵãfÂ+ß@qIáËa"@áIÈ î?Ñ~Ç[HÐÿ¿ÙÏUàW¿ßgçšÙ_­¿éb—oîM¿îàWÄ4?§i™v´UNASNone3FGL J1636.2-4709c?¿CqރrU?ǃz0Ñ6Ç?ì'Ä/'µ?ǃz0Ñ6Ç?άÈüÄÈX?Ç·Ý©§â?èTÍÀÎÍê?Ç·Ý©§â?Õ#9<íû?³÷ɳd\P?ånc{á‰?³÷ɳd\P?ÐË.ß]ë?µ@8 Í˜ä?çñšhQ
?µ@8 Í˜ä?¨Õö">?ƑBA1èI?îr Ÿ$ül?ƑBA1èI?"Ó2¶nc ?àU¬Û?ïafjuÈ7?àU¬Û?£åÝüáAÃ?™dÿv¿»?îÁ¢ ?ªT?™dÿv¿»?q&UŸò?i½>4§ƒ?ïݳUòÈ?i½>4§ƒ4PSR4FGL J1637.3-6325?¸ÎöîØgÀ%«ËÉdcÀ:¦°ÞY½À<!<(F@ý'_d@@@¡°¿P?ÒJ¢e›?Òò=ºË˜@ëó{??û0¬%~é¿ìîX}šŠ…?ï°*À¿ãOøØ¿â†ðY|s¿ïÿ']<9¿ïÀöÕ´ÒÛUNASNone?ïÄRv*ºÐ?…ôê³d1?}ÖÄá° ?…ôê³d1?îžÅj$Xq?¨ËIš÷¿I?¦©\ªí?¨ËIš÷¿I?î\wfê½?–@¹{1?ª8Ž'T.?–@¹{1?kOÃ?†ó+){-Ü?¥Õ©J~¸Ê?†ó+){-Ü?ï\cìl-?šgF=ڊ?"s'yY—¨?šgF=ڊ?é=ˆ:c?ʟ¾ÕEõ¶?Ëã	ß¾r?ʟ¾ÕEõ¶?늅r?«µÐlJž7?ÃñיëŠ8?«µÐlJž7?æShÎË?¸K&û†8?ÓYÓ/bj?¸K&û†8AGN4FGL J1637.5+3005?ï%¥šÈˆ@Dd| À:ãi:V=#À<‡CrE˜@ùrŸ.ÙÝ@~³¾"æ?ÆÕKÚt?ˆ ×üUÑn?¿Øš Õ£
@ÈYÖ5+[?ïü—`uÖ¿èNƱ¿åo—Òïü}¿è‰/žÔ¿ïö(°ù1°¿ßÚ{v˜ã'UNASNone?ï¶VÓÛE?ªR;CõcŸ?'jÀü·?ªR;CõcŸ?ïáÓÞlv?yU@´³ø?n,å)ҙ»?yU@´³ø?ï-Múùtº?"ÒÇ ƒ'Ç?šV@ Ñhµ?"ÒÇ ƒ'Ç?玲Š'¿?p³Ð'\Õ?†T¹HH?p³Ð'\Õ?ï½Á5˜?ƒ<_ŸªW:?€»Ï»réù?ƒ<_ŸªW:?ï…Y\MïÞ?œØ^ŽFMn?Ž©¨â54'?œØ^ŽFMn?ïïÅÓ¼ß?–Yۉ@?'?œ'Nj ?–Yۉ@?'?í~9L¸ür?Ÿîœ?9·?´5š8s?Ÿîœ?9·AGN4FGL J1638.1-4641c?Æò}ûZC?Ê¢œâú5¼À9·ÛàfÅÀ;`®­ýÔ­@ §è½@G'Ñ(| ?Ö©Q2!»<?ïÕÿ™'Ú@ò¶ä-;¢@&½cÎ0¥¿ïõ~̹­?ì!S6Þ¹^¿wõÚã¿äúf¼Í{¿êï…>BÛÈ¿ïÿåþÌúUNASNone?ë0Mˆ§Œ?ÂåþÜc¡?Ã>ÉÝaÎ?ÂåþÜc¡?èOxc>à?ÊD0['wç?ÎÂs´?ÊD0['wç?è¯ùPþ'?¯‡Ú¥3ë?Í@¼Çc?¯‡Ú¥3ë?ãD÷@òA.?º¡Þô ?Ùv~}¤?º¡Þô ?ÏKÖGÓ\?ÈÍøm7]?è-Šn)?ÈÍøm7]?Ùzª~vÜ?Ò'½oræ?ãBªÀđü?Ò'½oræ?Ü]Hñò‡X?·rí"
§o?áÑ[‡¼T?·rí"
§o?ÃW52Ph?³ÞAޓ¦?ë*2¼skæ?³ÞAޓ¦8MIXED4FGL J1639.0-2727?çÍgÚãC@)"¨ŸÆÚEÀ9ÜZ°O¾"À;¹¶à…@Y¤¼e@컚ua¬?ÃWq–ë?Áûÿ)ì7¡?üÖ$ê›í?ý['l×CÉ?ÏòpËD7¿â:7žÒ¾~¿æµŒt)¿á›>¤€¿ë¬`Eºõ¿ïÿÿ>¹úUNASNone?ïێ^RÕ?q8ÒuÂ?r8ÐÜqõ'?q8ÒuÂ?î¶;
Ы²?¨
"»ý?¤œO#Ñ+Ü?¨
"»ý?ï	-Rôn§?'J*U?žÚU¦™•?'J*U?ïpÇ=kÆ?}žrÞ¥*‡?œ±ç
U4?}žrÞ¥*‡?îZ}Œ?5l?°×~¶Ò*(?ªX'> ^6?°×~¶Ò*(?æåk8ïF?ÍitX—q?Ò5ã)Ž!t?ÍitX—q?ê#«Óz]a?´NÆyCY?ÇqP²Š}?´NÆyCY?èÍÑ[Ê"›?¯?(£¦ýt?ÌȺ×u•?¯?(£¦ýtAGN4FGL J1639.2-5638¿èrÜ×˝À+äøé‹À9ñ¿ä†ý¶À;¥0°¡óÛ@sYùñs@ÝڋÒ0º?Ê÷8[;:?áÉø;æ`@:k
•ù@n‡/×?ïޝåX´Í¿ÝYßð@¿éÕá"oA¿ïýð@o\¿æ)f–7Š¿ê°ßьO.UNASNone?ïÜHž]?¡¿6­®Q÷?Dvíì-ð?¡¿6­®Q÷?ä1¤'"j?ÊCJUlK¶?ם̷±»,?ÊCJUlK¶?ë‰QàóÊ?¦Þæ‹¢3?ÁÚ¸°0×?¦Þæ‹¢3?éˆá€cÈ?©E'R"'?ÉÜyþs¸ß?©E'R"'?ëYÜ׏|?Äš+:?›øŒ¡Â?Äš+:?¹Å½à†ú?ÂÛ!)×{
?ìÇHCï ½?ÂÛ!)×{
?âO?-glK?¼ßsûFÕ?Ûa¥1'j?¼ßsûFÕ?½L\†àü§?¯°^áo˜«?ìVto#àk?¯°^áo˜«MIXED4FGL J1639.2-0946?à¡% ˜H@7¡Â # –À:òþUÀ<åê«%@ òæ0v@°nºÈ¾J?ăùdo¿¦|c /Ø,?åKÕ@Ž»o?ߕ<¯« L¿ïí	î–K0?ïP3ôú€¿·Ux­eÔE¿ë¨F`®_¿án•Š¯œ?ÔÉÞZ鰈UNASNone?ï¿â‹u¤?«,ÞPõê<?€]8Š¡?«,ÞPõê<?ê‰¯ÇG?È#9|3¾Z?ÅÛÏù@âã?È#9|3¾Z?î—.´)¸?U;°ß?¦µu–{?U;°ß?ìŵh¤{—?£œ$1Nz?¹ÒTºÜ#F?£œ$1Nz?ï£/ÚkÏ?'c—
ª
÷?‡9´#|?'c—
ª
÷?Ö$"ïï?Óv'˜ôX,?äíþîˆx?Óv'˜ôX,?î‡øÒ¾'? Ù$ýnù?§€rã¹…? Ù$ýnù?Û°m‹s¼?Á£m££u?â'É:F!ø?Á£m££uMIXED4FGL J1639.3-5146?Ô¤FóÑÀÊÀ
©9û¤QÀ8Z"ÀÀ;0r›þΨ@J(KK?ÿ'%hoU?´Á6þCè?ÓÁêAÞG@ Ã{®Í…@­±~'­¿³1¦–,QÿÞAMÝÙd‹¿Ö]B%iq¿á罞±†u¿ê0[²®=–¿éI˜ÐEþUNASNone3FGL J1639.4-5146?"ºÏcíÑ?¥¤Ñ%äût?ï­ÂsœI?¥¤Ñ%äût?½<÷"
í?¶5û{?ìX|Á¾¢?¶5û{?ÒK,{Uƒ7?±¤yR™ƒ^?æÚiÂU>e?±¤yR™ƒ^?Ìü!ü ™Ë?±zʶÝÁ?èÀ÷€÷ٍ?±zʶÝÁ?nŽÿÊ·?wqgV`?ïáqä?wqgV`?Ž3®í¹r?'|5Ÿbö?ï‡1D ?'|5Ÿbö?¯Pä×­õ?ªðÒVÄ?î
ñ²N51?ªðÒVÄ?}­V—hËF?o¨ŸºÓ¢•?ïÄ¥S¨É?o¨ŸºÓ¢•PSR4FGL J1639.8-4642c?Ö<ë\ž«@¿˜ÉF"'ìÀ7Ÿb¶®}À9,5Ý1žÞ@ }Ö§œ@¸TÛ#§¥?¿÷w›BF?ÂVŠüñ}@";~[O²?÷õY"š&1?½ï¯aOÊ?îØTTëꟿçue!ÂÈg¿æ/$°¹pÏ¿ë]"3¿áHΙ«UNASNone?Ïô…²uÍP?Е¼sÒú?èޓbŒ¬?Е¼sÒú?ÒMÁÝ?ËT4#ŒæÈ?æýurY?ËT4#ŒæÈ?×߈é?–?·Æ­c
?ä;‹`4¸?·Æ­c
?ÊÍ»N¸?²™=«S¢·?éL',|y'?²™=«S¢·?Åd˜ÎmG?Íh"ÅͲ®?ê¦ÙÿÌd®?Íh"ÅͲ®? 4h¤o¦?­L4Þog?îü¹uÆÅf?­L4Þog?ӃÜýÐ?·í ÀÅ?æ>1ÿ?·í ÀÅ?u-›Î62?p|ªÍ'ù_?ïÕ¤ÈTu¬?p|ªÍ'ù_0PSR4FGL J1640.3-4917¿ïó‡^ƒ˜ü¿üºüUP"mÀ9(اÌbDÀ:½ž¥rð@úü¹úb1@B_@Ø?À½ÃÚය?Èú(Óo@	¬Ÿ›;ZI@,òý8%?ê6'¾5Û.¿çj®YÒY¿äH$[ÿÛ¿ä«@ "€¿é ¨¡Ê?ª¿ïÿª¥Z—üUNASNone3FGL J1640.6-4917?ì\éÎÌgˆ?Á7¤q±@?½±‰œÃ½?Á7¤q±@?î>"mR?ªêB¢""?¬Ù1n"Û?ªêB¢""?ìTž{3Z©?«¾˜òÌì?½[&e*¸?«¾˜òÌì?8Ñò?ˆMü˶Ã?§ŽW+–ùÛ?ˆMü˶Ã?Öϲjuê"?Èt˜Düè?ä˜&ÊÅ
·?Èt˜Düè?äR.Ç?Îþ¡[.ú¿?×[óÅ£Òq?Îþ¡[.ú¿?á@@YXÙ?»}bßÑ¿Ù?ÝõMNN?»}bßÑ¿Ù?âÇõ¹h"?·s£põðä?Úpß.Ø?·s£põðäMIXED4FGL J1640.9-5853¿åžÌ"GÀ a«°'ÞÀ:*‰*¶ŒïÀ;Å0[žŽ@Õñµd{@Èb?ÍJ|Pª?×	üʃÒ@‡$Y{œY?ÿv"¹ªÎ?珻"–$š¿Ó¯¿uÌ4÷¿ä•"¦óõ0¿ìL<"Í¿áN3i¹Ø¿ïáü^à¶UNASNone?ïàíuŸû?mGÒvõ ?o÷£4o?mGÒvõ ?î\†ûK)8?«DÑ1vË?ª7M:~?«DÑ1vË?î®#QÇP•?"U‡?¥Ê⯷?"U‡?îæ}Îp?'qó§ûH?¡˜."ÿ‰?'qó§ûH?ï?,GS?–ð6qF¸M?˜Ú|=S?–ð6qF¸M?â<ý)"Š?Ϥ|òÊ?ۆ¬Öüë?Ϥ|òÊ?è'EIL¿?³‡ZÊg?ͺë²ÚÍ?³‡ZÊg?å^Sks&Ï?¹ñ¯I?ÕCY)²a?¹ñ¯IAGN4FGL J1641.3-2908?ïÒ2x‰e@&—PÁ¹sTÀ9}'šy"jÀ;š™sÚ@¶Ó'7@ýÉÄڐ?¿ª:P³Ì¡?Ö¹;àÖÄó@'Q~wÕ$?øpkܜù?ší"á4¿à£À9 ¿è:T¤MR¿ë³݆Xt¿ïÿpž"ÀI¿ïóÛ._"UNASNone?ãÐæî=N?ʬPÿ)žè?Ø^2"Ņc?ʬPÿ)žè?Ñ}«q³Kœ?È8|?¸ôö?çA*G&Z2?È8|?¸ôö?æ惽ÂÌK?°Z¤Fî4?Ò2ø"zgi?°Z¤Fî4?ߥ4"–±n?±F¦?à-e¶4§I?±F¦?ÅPäßh/ê?Âۚ–ªâþ?ê«ÆÈ%ô?Âۚ–ªâþ?Ÿ+҃Õhü?­êÒtÁ?ï¡lNx?­êÒtÁ?Ôî$¡Ü'?´úIbÛU?åˆí¯ó??´úIbÛU?ŸŠ›*çï?ŒM®"nVx?ï«&›'?ŒM®"nVxMIXED4FGL J1641.5+2017?âü8­›"*@Bª\=îxÀ;ÃcTc.¤À<ÇÉ"a:@#gß?ùiþ†ƒ<`?Ë*'Wގ¿£à­Õ:Úq?ÚÃE¤ú˹?ü¡ô;ђY¿×Ɉ'N?è{½`H?4¿Ùu
ƒ'šr¿ÚÅéï'î¿Ùn¾ú|2¿Ç]ŠÊžÊ0UNASNone?ïüz$rë?9Wu½IÐ?<.á²â·?9Wu½IÐ?ïٗ¬À¤?o/©ä?s4)Ð9?o/©ä?ïàR'a5?qhÌ°dç¬?o­ØÆKB?qhÌ°dç¬?ïÖiFs4‰?c"¼"¼ý÷?tË\ÍDó£?c"¼"¼ý÷?ïú楈\¨?>½ª-#f'?Dejã"ò½?>½ª-#f'?ïnø—ðæ? #qðÄ^û?' ìþ~GD? #qðÄ^û?ïÞfåYa?wL[_6›A?pÌóTÃ?wL[_6›A?ï2T Ç(?úÙxÍ^R?™¿µ}žèî?úÙxÍ^RAGN4FGL J1642.1-5128¿Å^23ó'LÀ¨…·d†À9¼i"ïÀ:Ý(8-n@"v4åç@_­)™V~?ÒÊ"Ýtæ?àƂ@³½@e¼¦äÜ?ôÇ]_Áq¿ÕþŸb†\ü?íìk΅3±¿èIˆÇì=¿íX›7(‹:¿íÅý¥²­¿ïŠÐsJzxUNASNone?í«µk¿8?¾½ý&1?²¢WZê8A?¾½ý&1?Öºý^‡l=?ÐižÆ‹?䢁P¼Iâ?ÐižÆ‹?çÓ•kë?±"ϼy)?ÐYÖÕ()Ú?±"ϼy)?ÕÖQÁúÈ?³‹ïs&#'?åuל?³‹ïs&#'?ç¸uIÙ?Ï3$çãK?ЏlMÜ?Ï3$çãK?±³zb¿	b?¿Z"\¢B?íɐ³¨Ô?¿Z"\¢B?×ÈìÎk?¶ÿŠEs#?ä‰ò˜Êx?¶ÿŠEs#?'lÊ>1|?tè#û¿ÌÝ?ï¶O¬Ýær?tè#û¿ÌÝMIXED4FGL J1643.1+1436?åâŽm@ .@AuY_í¦aÀ:ÇÌW\À<8Íl.ýD@ßÿ|Øï@;ßY—K?ъ<6\?Êæc¡ºû>?õ¶¥ÉRÄÉ?ðûpú,?ïdH•:¿ç~(kBn¿ç$›?áíE¿æ "@º¿ïÿk*M±?ïú}¹©"UNASNone?î4Î#N¨?¼»Þ5?¬³'˜s?¼»Þ5?뽋¯Sȳ?ƋCøIʜ?Á	ÑB°Ý6?ƋCøIʜ?í÷£<R
5?Ÿù"䪸F?°Bæ·ÈW?Ÿù"䪸F?íRõß{â5? "JKéé?µhQF¯×? "JKéé?£eÜd?¯yZ"Ïýs?¦¦eËZ¾?¯yZ"Ïýs?Ó
ŠÔ.ì?Ñctïk2?æy}º•èŠ?Ñctïk2?êúç82<?±•R¦Ú¹Ž?Äc›7?±•R¦Ú¹Ž?Ùæ²³×]?ÀÛ¯B6M?ã¦÷¦Q?ÀÛ¯B6MMIXED4FGL J1643.3-3148¿Ü­³…g!@"|/øìÀ:‹O—ZÀ<DÂ<Pg@9!­NØ*?ÿ?èh3Æ?ʓù\!éà?ۅÎÁC¬¨@‰È]ÒC.@÷é¶9¸?ïôŽýß>i¿çö#]R@•¿ÄQj‹¿ÝӇ;žÍ¿íƒ9¿ïýPÃfò}UNASNone?§ˆð?¦ý•hBÅ´?¥ÕUŠ­?¦ý•hBÅ´?¯2?°>ˆ‹[;±?¯•dk9‰ä?°>ˆ‹[;±?ìß»û û¬?¢ù®bk"?¹ )ä?¢ù®bk"?îv»q–×Y?‡íàŒ?¨"H嶣w?‡íàŒ?ìÍs/™íõ?·
G…‹?¹"fæµÜ?·
G…‹?åP¶éᅗ?ή¤3?Õ^',<ôÓ?ή¤3?åFöñ°Ô@?¹sïèýý>?ÕržW€?¹sïèýý>?è"!ZBÁœ?¬èWª§W?ͯz–ôù'?¬èWª§WAGN4FGL J1644.1-3055?ԛN·ü@#d:æ…ÛÀ:&k/#:À;žM³9ä@ÙDÿŽk@í£3vO?Î,êâúâ?ÔÉÍéØ?ó›ªà?ÿ)µ@>3—¿ï8‰ÿr¼`?ïò)}§ËŒ¿ìJG¡Õ'd¿Ý‰LûoV¿ë³_¾V'^¿ïùVbã$'UNASNone?ïÂכ\è8?"´£H4›??~"2K\—×?"´£H4›??ï¯HÏw?¨W¢áéU?jöÆÙ3?¨W¢áéU?îiy½uÔ?™ž3Þß?©hd%@Ì?™ž3Þß?ïŸS¹ Ù¦?p"¾ìCp|?ˆ+¦›Šµ?p"¾ìCp|?î'"®«¤‰?³T&}˜1:?­Õ!žn?³T&}˜1:?é€Ä¸£—l?Ëw˜ŸÀòp?Éüíq¢Q?Ëw˜ŸÀòp?è¨ñMµ•y?´Þ$Nn?Í\:É)ª?´Þ$Nn?ë½¾žÙþ?°Q'tàfX?Á	"›¨	?°Q'tàfXAGN4FGL J1644.1-5009¿ïlÅgJ3Àž"B€À9†³k¢À:ïü£T-@££Ùäbk@1n¢u
n?ÓQ§àY?ÛÐo¼@I[»èxû@SóÈF*?³?¼X‹\j?¶8ÐÁy§¿ãRAK#êÁ¿êÞÊl <¿ïñà¸<?ízVs'UNASNone3FGL J1643.6-5002?ï˜d3õê—?£d
uâ Ã?‰æòø6†E?£d
uâ Ã?îõ;ƒŽÀM?¤_7f&X7? ¬GÇïâ3?¤_7f&X7?êO¯ÂÈ3'?­:wâDI?ÆÁ@ôß1÷?­:wâDI?îì,\€x?‰[z|?¡=>ìu?‰[z|?ëtæ*…©g?Á("ÿVû?Â,gUéZf?Á("ÿVû?å—LõüñÙ?ыó~<põ?ÔÑfO?ыó~<põ?â10þ¿Qÿ?¹:'2-?۝ž\?¹:'2-?â'I…u(?¾Ò~´Þ;?ÚÛmÈõ°?¾Ò~´Þ;AGN4FGL J1644.8+1850?ìà2u¦¨Ô@B
Š†×6À:¾B°Ž©À<{ˆÀ-'@Eïµ+?ý¤òÈßØB?Í[JiÑK?ÐÈ b‹l@ö¹!õN@ÊCt
¿ïÛ^g"d?饣'·Ôî¿Ñù1Øýˆ¿Îa
6u¿ênÂÀÚPC¿â—À±5—'UNASNone?ïÃë*—"?ƒ¾™B?~
jÕrv?ƒ¾™B?ï_žg£l?¢sX?ƺE?"3q´³?¢sX?ƺE?ïTŒ–ÎÊ?Š*!ÿ\?•nt^¯?Š*!ÿ\?îð¹n©´w?~°òž–? ôiøm…?~°òž–?îì>vՖÂ?›c?¾§ˆ)?¡<–/×?›c?¾§ˆ)?ít¤('™è?¿]C…™e?´ZÞ½¢þÁ?¿]C…™e?í>íœâ
?¤Rk¦¤ìt?¶—Š=´?¤Rk¦¤ìt?ëIYËÖá?­ïèAÞ¡Õ?Âۚ˜Ð¤{?­ïèAÞ¡ÕAGN4FGL J1644.9-4921¿ì/ñÎþšÀL,äd™À9@4ŠKGýÀ:°Ñ®³Ý@é.¦†'@
–»˜Çã?՘L};?ç}®ˆ@•ƒgþí?ú™¨	ôËn¿ïò°Vt€Û?ïýí@
¿ê\ܤZé¿ïÿøsCÄ{?ïÿKÚÉ咿ïÿþÐñUNASNone?îŽ}U|?ÁïAôß?®·*zDB?ÁïAôß?éB˜¤YÄ ?ÌPˆŒ3³?Êõn˜í€?ÌPˆŒ3³?åîÍ ‡I‹?³`~"5X(?Ô"d¾ñlê?³`~"5X(?î<!Éÿ?©Rl¬?¬=î5óÄî?©Rl¬?ê^mLšÊ?ÌÅN­{ès?ƅÊJ͔Ú?ÌÅN­{ès?͓w)	í?Ñz˜ˆ³©?è›"5½"¹?Ñz˜ˆ³©?àûB[o<y?¹âQ$}?Þ	{I!‡?¹âQ$}?Ðl:»½±?Ñ󓽃ûð?çüIâ¢!(?Ñ󓽃ûðMIXED4FGL J1645.0+1654¿ìvëÞy·@A­¸<òϖÀ;ÇvK¶¸À<s;ʱiš@á4"å@šoŊ¹,?ÏD¤_E_Ü?©ì^¤Ö?܄YÒÚ-?ÿN‹‰
«¿ÔʏZÑ\Ô¿é^`¨·CÏ¿áØa@Þ°¿â!†BNÚ¿âçÉ0`¿é$UIÞpcUNASNone?ïùWê͓Ç?C²ìÆy5ö?J TÔ"æ²?C²ìÆy5ö?ïå—²Ú*?uðõÒ¬??jhý#ê†j?uðõÒ¬??ïáZXĚØ?møüä>D?n¥§0fhT?møüä>D?ïâÞ÷x"?PÔYí\éS?m!üèëÎ?PÔYí\éS?ïï×z!?Y)Ï·®Çš?`(…ûÅS?Y)Ï·®Çš?ï'KnŠÄŒ?"–¤¯'ÎP?‹­$d.ö?"–¤¯'ÎP?ï҆ñ)2?}Éah¾Åú?v¼‡m¢á?}Éah¾Åú?ïIùj±ñ÷?ƒ²ÿæd?–ÀÒ¢â‰?ƒ²ÿædAGN4FGL J1645.1-4123c¿îÃò)
ü~@ý+9i®À9ËQ•	ÖÀ;R"nmØ@ â"ÊZW@œ	€²B?Ȕ¤ý¥Ý ?ÏB¨Ã
†@‡p_
¬'?þà-,3Ë?ìÖ`^åh¥?ïâžá78¿Ü=oa·ªý¿Þ3.€›ñ¹¿êãs¢¡¿âüýKð™[UNASNone?î[àjRH?²st	õÊ?®jAüÊwz?²st	õÊ?ëGÅ<#Œ?½æ‹á[`_?ÂáˆëqÒ?½æ‹á[`_?í´3I?W? \·ÐŒ+?²^eµî7K? \·ÐŒ+?ìÓ;HLí?¡]ω­£?¿af%½˜–?¡]ω­£?ä	Î>«¦%?ÅáÚá ?×ìc'¨³µ?ÅáÚá ?Û,Aœ''?Ðpòe&%?âi¹_1¾¿?Ðpòe&%?á¥cߣi&?º\{ùB ?ܵ8@¹-´?º\{ùB ?Ü̺oõRÊ?ºû¶'™g?ᙢÈV›?ºû¶'™g$MIXED4FGL J1645.2-5218?ÁƒßnÌ!½Às©óƒð»À9¼)DœèÀ;/Ââæ@»ÑOéL_@&t	?á » Ôv?Õ¡}]ù°[@(a´Oþ@ÍüLÂ%?ïüÒf(S¿é1ÁXÐQ¿ë¯¾¿Böu¿ãr®]Ëã¿ïòÔÔK4¿àME}¸'ƒUNASNone?çXß'^?Òj9bTç?ÑNAûç±C?Òj9bTç?ê®óîyÅ¿?Âlò?ÅD0Fé?Âlò?ì2<Ƹi?§
ËœâR?¿fnÊ<¶?§
ËœâR?ìpŒ=¡²S?Ÿw˜>À?¼{žòmh?Ÿw˜>À?Þ×zÒÑk?ÓºJw%.?à"B–—Jy?ÓºJw%.?ÑOYçIr1?ÐDÏÝùDû?çXS[Fç?ÐDÏÝùDû?á!‰¿ÔË?¸úÞzX¾?ݼìÀVi?¸úÞzX¾?Ë1WÂDï¯?µu8·z¬Ï?é3ªnÄ?µu8·z¬ÏMIXED4FGL J1645.4-5514?æ2&
À*è},{‰À:¨`ÔV.À;ÇÌÒ¬	ß@HýwÞ@DÄ¥¶ÞN?Ԃ¡z¹"œ?âövÛ)@©G{¿"@Õ†å"?ïç''kþ¿ãPR]šåÊ¿æk_)[C¿ë˘_1鲿ïÿÿ" 5•?ï÷üß¶´UNASNone?ín">]!³?ÆaGý‰qó?´Žî`Ìç?ÆaGý‰qó?ím/>˜?º‹8$V?·G˜=Ù<?º‹8$V?ì¶úÒ]t>?¦+Rx¤ªº?ºH)m^?¦+Rx¤ªº?î–Õ¤·¯Ú?'ò†nhˆ?¦'¥±ñMa?'ò†nhˆ?éÁ8¥@Ÿ`?É©; óˆ¬?Èûjý'€?É©; óˆ¬?Ój¨ª{?Ð>"_T	©?æJø«ð*Â?Ð>"_T	©?âÎäª0ð?½²¿<bÔ-?Úb6«ãž ?½²¿<bÔ-?ÝÖQLñÐ?Á'ì{`?þ?á×Y‡t˜?Á'ì{`?þMIXED4FGL J1646.5-4406?¨3(<ÞMk?éÀ̾µÀ8â­Yiþ¡À:PÑCT§@#úäY€@²¤}"jŽ?ȸ=³™?Ã5֟™?ü¸n;Fýë@ã[:¹9r?ïþôÒ¥Sâ¿å—ñŽM5=¿à',)S¶`¿æj*sq¿èï€@'&5¿ï딾h…ûUNASNone?䤻"?Ñ̆¡jµ?×î·ã܈×?Ñ̆¡jµ?î>A@HV?°`'-lþ9?¬î"¥?°`'-lþ9?ãÏ €ù~?¹R2¬?Ø`¿Êþ
?¹R2¬?íù9|Î\Å?"{´~zÄ?°64iØ?"{´~zÄ?Ô¨hêO>­?ÎãéœÄÏÜ?å«ËŠØ`ª?ÎãéœÄÏÜ?æ¤(â*	Ç?ÎJÖÙÒ*?Ò·®;«ìq?ÎJÖÙÒ*?ág$É&é¾?·ùPC9e§?Ý1¶m²,…?·ùPC9e§?áeÜ'ޖN?¼YäÉ~õ»?Ý4G°BÓd?¼YäÉ~õ»MIXED4FGL J1646.7-2154?ïýòñÆùœ@-ÑÌÙb…À:°«."À;a_–i@6ãtt@Z¹ÚÁ6?ÈjkØLˆ?ßGX"%"@3̼ܔÁ@ ŽÂ%?ïÿ¶~¬®I¿á£qõáõ¿ãY.¥.ù¿ê!ÎAÒ¿êՀ?€sƒ¿ïþP½Ý›§UNASNone?ée{ò꘻?Äwø¥:.?Êj4U?Äwø¥:.?Û<zø¢FD?Î7/¢Q?âaƒ®ÜÞ?Î7/¢Q?æs0«= ?²3ĕ«)b?Óžä©"Á?²3ĕ«)b?å*@àÙ?±•%—qœ?Õÿ«~?îO?±•%—qœ?ß}N˜GÀ?ÑÝv'	…Ã?àAX³Üw ?ÑÝv'	…Ã?®€Æ )G?½዆í?îó•þl?½዆í?Ë÷&±"?³!Pã-ž?é8:öS·?³!Pã-ž?­P©0}…Ä?°êF™è*?î*õlܪÄ?°êF™è*MIXED4FGL J1647.5-5724¿äñ`̸CÃÀ˜Á@§üÀ:
·­€×+À;­ŽŸj"ó@¡Öiƒ§?@*~áS?Èz€ú'V?À¾ß8à^?õu°Ðî?ô¹#ØL\Ð?ïûÅs<7¿¿âc'·Ôî¿çº‹·XÇA¿ìõËß	¿¹HÄiüÉ¿ïú¤£|UNASNone?ï¹À•?²WøǶê6?¼ü@GÎ?²WøǶê6?îø¿¾'˜?ª)ˏç½_? ´‡ru?ª)ˏç½_?ï(SÃ/?'ØŒ˜™?šõœA6"?'ØŒ˜™?DÉ;P?vRœµxâ[?Šý?vRœµxâ[?ï‡x*Ó@?'í¼L6—?Ž!õ{Ë0?'í¼L6—?æéF,V—‰?Ï(8G3	?Ò-s§RÐï?Ï(8G3	?ìÌ}{ï1?©VS~H†?¹œ< †w?©VS~H†?és¸U'¥?»ÆS»,Ö?Ê1Á©õn?»ÆS»,ÖAGN4FGL J1648.1-1547¿îy¹N'x@2Y"9ÞHÀ:'÷†®À< aïß Œ@"tX€Ÿ¢?ûíÄÉÉN?ÄQÚþ"ÄC?¢ÎéõÒ?á#œ½:ˆ'@J†áÛþ¿åµv9B@í?ïý
q؊p?Ô÷dÛ¡Ò¿àä#á0±ú¿ÑWÊ¡ú;E¿Õšü›¤ÌUNASNone?ïè•_ož–?w@&8Ð?gj ¸<áù?w@&8Ð?ïÈ×&íՆ?ˆÆ""ŠýC?{"lq·å?ˆÆ""ŠýC?ﲏÔô¹{?"f–²r6?ƒ\
ÁÓJ?"f–²r6?ïÓÏóë?b揮˜¶?vx˜'´º?b揮˜¶?ïÎ?jÆiÔ?}OÀ)7?xàJ«9r?}OÀ)7?î3 ýwJË?·Lÿ*…?¬Åð%·N?·Lÿ*…?ï/	¿?<³rZPß?úÈÇ?<³rZPß?ïŠéMŒG?ÀRçÄk?Eºå½¶9?ÀRçÄkAGN4FGL J1648.7+4834?í9ФÙÏÑ@CúúaZëÀ;mÔZ_ÇçÀ<Õί%@)K'Mð¤@Y{2¦E?Ӟì>Ø
?ÁñÞªïj?ò^/`?Û¸?þüE2º‰?ë{¥BDH.?çaR*o?S¿é!³äžzª¿©š«½]™
¿ç`{~¿ïþÜÇÔUNASNone?ïú\…!f?Dï™ÄT:—?FëOZþ?Dï™ÄT:—?ïÅ¡ŠÝFË?ƒ—;D‡I?}/:'î>…?ƒ—;D‡I?ïÛvc3«ÿ?nÙÁUð¬?rDÎPÜl¢?nÙÁUð¬?ït¯¡1­;?u¬¬QEW¤?'jØŠ£?u¬¬QEW¤?ïÕ½‡ñŒ±?€¤¤§"?u!<Y/ˆ?€¤¤§"?ïîpØt?¬'¥®.F?žâ,K¹ˆ?¬'¥®.F?ï'1™ç-‡?ŠÚ4ù¸¼j?‹³™"ó?ŠÚ4ù¸¼j?íXý÷ßl"?¤4Ãw«¶'?µ8@(´á?¤4Ãw«¶'AGN4FGL J1649.2-4513c?á¢F·}ú¿Ò¯¹Á'@âÀ8!:жfYÀ9'˜³ÀŒM@šô¥A@ÍãÉª?ÉS–€	¥›?×D¾uñô¥@úúr!…Œ?ô÷öO½¿æÊUŽ§Î?î‰IõíW‡¿äwv#rËÏ¿ì
"¸aþ¿ë*e~ßÙð¿ïÿø]Ê5™UNASNone1FGL J1649.3-4501c?Þ8&óöŸ?Õ}Ý»ÝfM?àãì†{"±?Õ}Ý»ÝfM?ÃFfv'?¿
"ݶî®?ë.fb_›œ?¿
"ݶî®?Ù
ªÞ»ü?µ¶!BM‹?ãy*ÿ¢?µ¶!BM‹?¸Š	e¦ÅI?¢"ߨò}?ìî¾ÓK'W?¢"ߨò}?ғ 6Òá?ÖÎ{6	ÚÓ?æ¶/䖏p?ÖÎ{6	ÚÓ?Â˜…"ý?– "ì0mÆ?ïyë;LÝ(?– "ì0mÆ?·'º2d'ì?§ôƒÕý‹?í
¨¹êib?§ôƒÕý‹?SR鑓©?Ié<'ü-ð?ïöV‹y	?Ié<'ü-ð8PSR4FGL J1649.3-4441?ÆYgÝÅ?¡Uûà
Â&À8š³zoÔÀ:6¥Nفç@xF(XcÄ@'I†\?ÄƞµbLü?ÛÒF‰QLú@Þ¶¿DN?ñ#3¾ÉSñ?ï$'¯ÀM¿ÓÁþ\緊¿ÝF1\ïDF¿ä8Ÿž–Xœ¿ìŸÖjÛ@¿ç,ÉVö†ÚUNASNone3FGL J1650.0-4438c?©C]2A8?¹2îÍè?îkÊ,Î.?¹2îÍè?ÁùÀ&?»¹ÓÊ?ë¾Aþvy?»¹ÓÊ?ËqŸÛä(?°Ÿkó•¥?é#˜	õú?°Ÿkó•¥?³Y»zÛa'?˜:Ò½·
?í"Ȑ–Õ^?˜:Ò½·
?'IóŽä|?ºMÓrƒU5?ïu°c_ Ï?ºMÓrƒU5?‹:»{^ú?'®ŒÇƒt°?ï"–"?'®ŒÇƒt°?žóÜK¾ñø?'Zè4Ût?ïa¯Æà?'Zè4Ût?[Ze Ë
?JtsûM?ïò}ÒØnZ?JtsûMPSR4FGL J1650.9-4420c¿ÒlbÈæÒ÷?£Ú"1`ÔÀ8W-À-À9™™ãktÃ@A0êX£Û@ª¢]yÑ?ÍZ@ãÉ?Ö®F#û²¾@"gÁLf@.Š:ÖëŠ?ï÷õoƒEš¿á^ÛÝáÈ¿â·[ÐKÝ¿è°é¬×d¿ïÿ{@>Ç?ïŽXÐàÙUNASNone?á",ŒiÊ
?ÕÔAòO?Ý»¦ç,kæ?ÕÔAòO?Û´WnœJ?ÐÐ{؊è?â%ÔHþ1Û?ÐÐ{؊è?Þ3€»É'?¸}Á•ÄÊ?àæq?¢7?¸}Á•ÄÊ?â
,'Œœ?¼µÈÆ¥7Õ?Ûå¦ÜçæÈ?¼µÈÆ¥7Õ?Ü	j4Ú°Ä?×5OZä°¢?áûJ咧ž?×5OZä°¢?£‡˜»æ?³ƒFü%Æ\?îǎf''?³ƒFü%Æ\?Á£â¦[|†?¬
æÑÅTê?ë—Vi Þ?¬
æÑÅTê?•¨Ê­ñfö?Mm˜¿b?ïR¹ªt÷è?Mm˜¿b<MIXED4FGL J1651.1-5848¿ïó&äáÀ"Op\‰À:lm¥À<Lï'Êr@eÂõ]¨@`¿B Ž€?ЬbÉù´?æYYø™Ú@l¯c/zA?ý‰oG‹"Ù?é(j¢‹/ɿޘüŸ£I¿à|·áƒ=7¿ïÝEö"V;¿ïøï4Ö¡b¿ëwž!"£‹UNASNone?魎Øí¹Ï?ÄnÖંÔ?ÉIĜIÅ?ÄnÖંÔ?Þ>ʞ§Óø?ʜ۸¢ô6?ààš°¬?ʜ۸¢ô6?æ$ƒÿÓF?²&KåõW?Ó¶øÞYu?²&KåõW?á†,ôø"?¯D¨Ÿžõ?Üó¦òø?¯D¨Ÿžõ?Øso4&‰h?ΛM¦Hv?ãÆHeì»L?ΛM¦Hv?²juéIæ?¹Ñ.YkN?í²±B­¤"?¹Ñ.YkN?Ëş.ât2?°9á	?é˜4Gbô?°9á	?¯…íž?–ó·Œ¬û?î®0ï%?–ó·Œ¬ûMIXED4FGL J1651.7-7241¿ÎõøN@«À1§õûmÊÀ;–÷ÎVòÀ<·•XÂ8õ@!MþºÞ?ÿöÊ,œ‡?Ë9\˜q‰¿~6¼ïMð?µW"ðbS?ñå_?ք²?îvŠÖˆ7r¿âì½B–'Ÿ¿ÜÄр»§6¿äM²À²W¿áf—éJ¿Ó®,ƒk¯ÑUNASNone?ïü¤ÐѶŽ?8ê¯8\br?:Ùzؼhd?8ê¯8\br?ïØE«¨1Y?âÖ2«ë­?sÝ*Jë|?âÖ2«ë­?ïàüë´ª¨?o–^YZAó?o~/s?o–^YZAó?ïÛT=U1F?W¬£ë	×M?rUá_¶0ð?W¬£ë	×M?ïû½—"u‡?GbÐCŠÝ?A	¢€+›¸?GbÐCŠÝ?ïˆÉÄþ{? 8Œ?g>Á?ÍŽóá)I? 8Œ?g>Á?ïÚ:=q-?yæåuÍ?r÷âÀK)Š?yæåuÍ?ï=Ãk5i?P}ü-½?Ÿ˜G—À¼Î?P}ü-½AGN4FGL J1651.7-4359¿ã-íÞDÈ?ÃsÖuB!À8Él4Á
À:?u –
@†«×‰¿1@÷n¾ú|3?̂®›‰]â?ãD:AšT*@³Bؤ@8…a8ª?ïü7ž|ØC¿×)íÍ:¿Öª9DDR•¿æ%Ž?w4¿îrg'Ñ`¿ïÿšÜ|UNASNone?®§Þ	щ?¾§Õ'ºK?î†!ö'˜?¾§Õ'ºK?ÅgÀY??½K?å,Ú?ê¦ùi°??½K?å,Ú?ËÜ´1±?°.¼;f$Ñ?é>Òó"œ?°.¼;f$Ñ?Ä؆ËgŒ?§™n`羙?êÉÞz
&?§™n`羙?ŠÏêP¥¼?¯¾=9v?À-'?¯¾=9v?ŽºqÃìÑ?"fÍf/l?ï…<#ê?"fÍf/l?©r{å­'?™8
?îhØAÜ)?™8
?vsÀÝæ?eñ¾¯äÅÎ?ïÓð—d?eñ¾¯äÅÎPSR4FGL J1652.2-4633e?î­»×~xù¿ø¤ˆxßæÀ6ÿÓÚÞˆÀ:4
*%mx@!?%Ó¤,p?þ»Q•	Ö?žBSŒšÉ?˜€k˜¬p?øþiâò¨ÿ?û~"æ+˜Š?É¡î&ä›K¿Ñ(›@¸­¿Þ•ƒÑF¿ÜIøœ‰c¿á–2§9¿Ûdÿ§j"UNASNone3FGL J1650.3-4600?ã¾?Ëh?ÑíÇ
›)?؃ہÆi0?ÑíÇ
›)?îMOy9ý¨?ºŠsK|*H?«+j¨W‡?ºŠsK|*H?å$¢ÝÌ5?µ»ñ˱Z0?Õ϶ºDg—?µ»ñ˱Z0?êI/ ùה?¸",ÿ×*
?ÆÛA|¡¯?¸",ÿ×*
?ä8éDk"?Îe¼ê¤?×ێ-w(ù?Îe¼ê¤?ë6tCáè?ʞÈ?ýς?Ã&.óˆx_?ʞÈ?ýς?è7^n¨Ý¸?¹Ðù3?Ï"†E\‰!?¹Ðù3?à•(4–N?Æù´G•?ßâÕ¯–Óc?Æù´G•AGN4FGL J1652.2-4516?҃a_|£{¿ç—MYO&¯À8¶lCõùÀ:GHÕ[ç‡@Ø èØÇ@¯ð£kªs?ƏêÄ.˜š?אջ2ño@'ö@c^@Ç&)àN4¿ë.ñºÂß
?Ɓkdýێ¿á)à¾ò·¿éA 'oÿl¿ìàD]ýâ¿ïû.¡UÑUNASNone?Ìͦ©
à?Ξœkc¯?è̖U¹½H?Ξœkc¯?Ü2dÅì"?ÍH
dþ™?áòf͝	ï?ÍH
dþ™?ؽï'Êr?µyåܝû?ã¡{ˆ6šÇ?µyåܝû?ã¸O±\ó?´:h¸y?؏`Fà?´:h¸y?ž%ÐÞ¥y?¦®$<¶™Ï?ïÑy&Sô?¦®$<¶™Ï?«{x$Ýh?¶¶0šB?îHHv;p™?¶¶0šB?²˜Ì[Œ
'?¢¸	3iëª?í¬ætW"?¢¸	3iëª?§þõ¸Û&¢?šÞŸTóO?›ˆæ?šÞŸTóOMIXED4FGL J1653.0+3640¿ïùÀ
ï@CW‹'¡¡À;¦±RFÀ<ÿ>Dß-"@Á¼.™ñX?ïö¶À›æü?àã¦Î5'™?ïöÌR֒@Šc0Q¤@~¼èS;¿åf3:¿ïo¿ì©õ÷¼e¿´3'J댿Ç–ý]
w¿ïüÙ¿úVs¿ïð²…"êUNASNone?ï¥3]Ðj¼?ŒÓ•€ê«?†³(\å?ŒÓ•€ê«?ïUdÆ?¥Uˆ½fBù?•N]Ï÷¡"?¥Uˆ½fBù?î:½14'"?˜¸ª"g"?¬T,éGJÐ?˜¸ª"g"?íå!rœ?œ#nué?°Ö÷Ll"?œ#nué?îvAýȺ'?¬ƒÎ+G?¨›à&ãòî?¬ƒÎ+G?î&V›Ã'?½:`'Ö ¥?­š–H9×?½:`'Ö ¥?í{ìó¼Xi?£ª!0/?´ ˜cg6?£ª!0/?ì"e…•×?³aøXë¥?¿&ìÓÓQK?³aøXë¥AGN4FGL J1653.2-4349¿éØ©H}2?­‹ÛàùïÀ7œƒujæ(À9Žß‰gó.@@éTA÷@=¼>	P?¹{'G•Á?Ҁ¿®Xë@´û'Ã@æb I?ïþ'ÍzÈ?ãm¬átú~¿å—˜mI¯v¿çךÈÙ"¿ì'†!퐒¿ïÿ踻ÐUNASNone3FGL J1652.8-4351?ªTÎe2œ¦?¼a'Ú?îZ³ÈS?¼a'Ú?¸Ú¹³59,?²ºÆÈ5jC?ìä¨Éb_?²ºÆÈ5jC?ŬsK¸?±Á[³z®V?ê"ÿã>m?±Á[³z®V?Ÿ'q—™z•?ŒïSGkG£?ïìs'·K?ŒïSGkG£?¥°ºKڍÄ?Á…¹çn0?î¤ôZýžô?Á…¹çn0?‡ý«ž,?Žqw_´¥Ì?÷?Žqw_´¥Ì?¢¯ÿb{i;?˜NEH¹¡/?îÕ	æÜ?˜NEH¹¡/?3è§'—Z?,ÊK?s"?ïý'ë4õ^?,ÊK?s"PSR4FGL J1654.2-4907c?µÒ	ú4!
Àe¦$ÂW(À9ŽX«'ÀbÀ;8òòÑCT@ÉÅjØ»î@ˆ¸»Ð`?Ç>ž¡@?Ä÷£‡?û˜…+•°@ !ÂG³¿çíeÿ8Yä¿èÛ­À˜$¿ç]Å]l¡¿ã¿FÒLhŽ¿ëe#ÀÏhˆ¿á¬åÁX¨UNASNone3FGL J1654.3-4907?ïò(¸Bž?^K	ññ©?[®ª?t®?^K	ññ©?ïہKë;?$Âߐ'D?r?qQf'?$Âߐ'D?ïx™
õ¦?ˆÚ%û½%:?ìßfØQ:?ˆÚ%û½%:?ïåbgJ´Q?Tƒœµ¶c?j˜é…¿?Tƒœµ¶c?ï]•¨&û?—µ DàX?"MJþ¯\Ÿ?—µ DàX?îðËrëÁ?±Ø~~? óHÒÕ°?±Ø~~?ëƱÉLuá?°.u#,?Àå8ÚÎ(~?°.u#,?îß(Jˆ°?"H•ï5Å?¢
{Zí þ?"H•ï5Å"AGN4FGL J1654.5-5509?ïÛ¦"ÃÀòFà!qÀ:6ž«QRÀ;˜14@î—\R'G@Ž÷!4-.?ÔU#}³Š?îÒ/w¼Ð@å?À	oë@ĆD}2†¿ßÇ7a–
¿ÙVÁãd¾Æ¿îˆ™A/R¿Ø8ÄA¸Ý¿î?²{è¯?äÝC!½¿êUNASNone?ìȦ;W?Á~ñZ†ð?¿ŸáºÎ%E?Á~ñZ†ð?ê;T—†ïÉ?Ħ‡h¿‡?Ç­¡ä@Ý?Ħ‡h¿‡?ê¶AL^J?«Å!ò>‹?Å&ûŽÎ†Ù?«Å!ò>‹?ì`ô|i2?¤ãßÜöšä?¼ø\¶o?¤ãßÜöšä?åÖöþ	ìÏ?θ¡¸ˆ-r?ÔRì&b?θ¡¸ˆ-r?ÈZâoõ?Ë[þñ°0?éø)G¤?Ë[þñ°0?àîœY"Â3?º-ïžÖ;Ù?Þ"ÇMº{š?º-ïžÖ;Ù?ÈhG5¸bv?¹*t_Ö
?éåî2'çb?¹*t_Ö
MIXED4FGL J1655.5-4737e?ïj"êÏ°òÀ@xw
À8Ý/n'"šÀ:ö´°¨ª@ €üU¦z©@¬ŒUÜ?¸.ðƒ`G>?'
ÛéË5?ÝüÙ·–Û@|²>¬
:?êؕ›^–¿×þí›ÏSæ¿éÖt`¿à¦"Àä¿Ý@€Cdô¿ä2Wk!UNASNone3FGL J1655.5-4748?ïî͎ÏÍC?^¶i²˜è?a2q\-¼H?^¶i²˜è?ïÙÿ2Ù#Ñ?ËÞ?"Ýò?sf˜íw"?ËÞ?"Ýò?™½½?›¨GÔ¢Pš?¥çÏyÓÀ,?›¨GÔ¢Pš?ïÎ^ñ`Ö?cœÅ©³U?xÐü›í<÷?cœÅ©³U?ï¾8¬¼.?žÌÓ>CÛ?œ(8êhzN?žÌÓ>CÛ?ï'«¨îSä?¬çëTTô'?›
ŠÝ?¬çëTTô'?³«¾Š? _†W°\?§F´Ç×ÌX? _†W°\?ï'¶{|£?Ö¡HåŠ?Ÿ-©7o£"?Ö¡HåŠAGN4FGL J1655.7-2411?뇚<4@'ºYÀe¶=À:mˆXÿvÀ;áÐ>qT×@†+<™¹O@GE‹$Œ?ÒÌÌ¡Ù¯?Ñ}	@¢C@kõQPT¬?ñÙ5©Eµ?ïþ;9'ò?©2­ý(à¿éYe5
ÿ¿Ø—9¢¸ý¿ïÿë""i·?ïúY,ÁÿêUNASNone?ï½Ìß?'°0IŽ?€Œø6Þ7?'°0IŽ?éÄþÀBƒf?È8úaI_ß?Èìþõòi?È8úaI_ß?í޷ĹC?œ7NàmÓ?±
Aؤm?œ7NàmÓ?íÔ:wÓ©¾?˜¨c<䂎?±^,CˆsŠ?˜¨c<䂎?îç« Õa?¯ã—ùã.¯?¡…MöÂñ?¯ã—ùã.¯?Æd*™S&?ËaÔÆÁE?êfõY«9w?ËaÔÆÁE?è«0ò¼?³€twùÐ?ÍS¿<7á?³€twùÐ?ݎT¦`Û?¾¦	Âo"?á8Õ¬øϓ?¾¦	Âo"MIXED4FGL J1655.9-3940?ï0úÀYŒ@@®I#`À9oe5
ÿÀ;
w?Ò}ç@Dl›ßš@ۉC
@Ì?Í58[' N?Ԟ$c½ù@%XdE#ö?ûqo´Bè2¿ßÒËÿÈLµ?輸dÉ®4?ÓS]Æ.οæ7ûþé¿ç®¤"‰—Ä¿çºßr#UNASNone?îmBPåÿ+?´.ŒJõž]?©+ÚïXL?´.ŒJõž]?éý'ÏӒd?ÂÕÄÒZ?È	ôÀ±¶q?ÂÕÄÒZ?êRŸ¬z"=?­ï–}êÃV?ƵN¯?­ï–}êÃV?é[  VU?®_6 —]?ʑí~¦­?®_6 —]?å—5Ó:hö?Êsê'>¾?ÔєY‹.?Êsê'>¾?Ør1þ]q?Ф¶Ò©I?ãÆôgÑG?Ф¶Ò©I?ä±bQó'?·Ï'K"žò?×à;\ý?·Ï'K"žò?ÓË/5D'?»k"!‡?æršhe]í?»k"!‡MIXED4FGL J1655.9-3101??þ6–@šºŸ¹À9óëƍ«À;•ËWÇ@Ë…$@22'3K‡?Êáž@zµ?Òa]¿îî@YP%²A0@ûÅÜ¿ì]ä·¥?ï¹ý‡»¢¿æ!;¹êqù¿çlÁÊ:K¿é|0¿ïø0þ¥ŒíUNASNone?ï¼_™î~"?}ÿ´ý<r?€èuB/y?}ÿ´ý<r?ìHlGsS?»Ÿvʯ?½¼Äec÷?»Ÿvʯ?î2Æëê}?˜
ƈ_?¬ÓŸmѼ6?˜
ƈ_?î8fQ©Ò?¾¶÷‡è@?¬yšâÏ*'?¾¶÷‡è@?ìö;­Íz"?·"Äv½T?¸N"'&7à?·"Äv½T?ÜCÝÙÿ)/?Ò5ˆ'?áÞkh?Ò5ˆ'?⁎Þ)Áo?¹2¾tÑÌ?ÚüâC¬}!?¹2¾tÑÌ?á¡6.‡Ÿ?½%3Õ6?ܽ˓¢ðÂ?½%3Õ6MIXED4FGL J1656.4-0410¿çÎg­Ÿq0@7.¡ ÏÀ:µ¼åÎüÀ<Š
RiY`@c
ÔoX}?þÛ£"Ń?Ì­3ªQx?ä) öÍ1@X§ç:6]@+C&E?ïÿ0,µÿ¿ç9Ù	ññJ¿œ9ÄØó²Ñ¿âž€ô‡%ú¿ëS—tü+¿ïü½àö¥cUNASNone?ߢ'!®Q?ÍV}¨nÁ?à.·po(Ø?ÍV}¨nÁ?áfÔ+LF?Ì+á¿à?Ý2W©gËt?Ì+á¿à?åX'Êuã?´–ÍY·Ý?ÕNÜk9ã?´–ÍY·Ý?ã@Ïq…Š?¯BÙ»À…?Ù~aÀôì?¯BÙ»À…?Êô7ÕVg?ÄÃÃÓmÀ?éBò8ʪf?ÄÃÃÓmÀ?ÀÝ'Û2¸†?ÅOÁHà¯?ëȶ	3QÞ?ÅOÁHà¯?ω<4
Π?´soú"ùT?è°òüŒX?´soú"ùT?Æà*F®?°Z´
…œ?êGú5nTz?°Z´
…œMIXED4FGL J1656.5-2733¿ïÿúÉVÂý@#Zï
å6PÀ:ŽP±É;HÀ<pSó.@ªvºœs"@kXZ4?ÍOʘ•Â?éäjþ{›'@4,ºËC@·dÒ<£I?ïÿ0ýñˆ¿è‡¤Ú?|¿³çÆÎ0$5¿ç¬—7¿‰î¿ïÿàŽ¾¿ï±g¸ÎéUNASNone?ÙQ4لå?͎¬¸|«?ãWe"=ñ?͎¬¸|«?ÑH=85Õ?ÆÇC¶c(ï?ç[ác÷e?ÆÇC¶c(ï?ܯÐßùG?²óá´jŸ?áò(]?²óá´jŸ?Õõ:t^æ?°¼®¬N?åxbÅЍ?°¼®¬N?Ų|æÚC?̲VÅÅ­°?ê"`Æz‰o?̲VÅÅ­°? j+ÇøàN?­Ète'ü?îù]CIx;?­Ète'ü?Æ@²ë­Á!?¯;œéa+?êoÓE¸?¯;œéa+?£o§Fš2?ÎÄÔ!?îÎy‹–]?ÎÄÔ!PSR4FGL J1656.9-4814?ëÌÞvÝçÀ	½nŠø'À9Ã;òõU'À;[;¸Ìe@UM–
îÆ@vßîÁ?Ö;Y½‹'C?ïNÀøƒ3ý@	 Vßà¥È@‹~M㸢¿ë}	@¢C¿ËßýV,‡r¿ç%IÑiò¿éŸ}ß(ïã¿â+úú݁P¿ïò¾UNASNone?mhkØ?¢Ôù:?Ì1?‹šä¬ÄB?¢Ôù:?Ì1?íøý
	ø?´ØRZ‹_?³8‹—A?´ØRZ‹_?í×±˜D?£4¶®çÚP?·ÁBvVß?£4¶®çÚP?íUw
 .?Ÿ~Ú=³È?µTGŠå?Ÿ~Ú=³È?îަޝüø?¦u-"çÅ?¢'ü~?¦u-"çÅ?߀
4#¦¬?ÓJ!ÂaS?à?ùeî,ª?ÓJ!ÂaS?ç%­l½Ì?²ŠBmö™?Ñ´z¥&"h?²ŠBmö™?Ø—Ùò?ÃpE\ô?ãð´~ž'?ÃpE\ôMIXED4FGL J1656.9-5717?ǾHoÛZ.À!¤Œ?>qÀ:¬TƒåÓ.À<+óV¤Q"@=lè5³ì@ij­?ÑAǀ\±²?âȘ?|l¸@,ûõ@þè'¯q¿ï¾´ -œñ?ïï* ­Ò¿âî1× ì¿éHÂ:¢"¿ìŽöþN¤ÿ¿ïÿ¦¶tFUNASNone?ëQ$_RBd?ÀÔGNÉ?»n'¶ön?ÀÔGNÉ?í5'_Zp?´'e…¥LÔ?¶Sí?´'e…¥LÔ?êË1'6¯?¯ƒ¯kE§?ÄÓ9÷%C?¯ƒ¯kE§?î4*'?¾›ùə·?¬¾ÎõUˆò?¾›ùə·?ßD,•4Z%?ЎÓÔEÏ?à]éµeÒî?ЎÓÔEÏ?àð$ÃXÚ¸?шv9JØ?Þ¶yNJ'?шv9JØ?ѪÒBÛ5?¾úÎ<Ç?ç*–Þö'e?¾úÎ<Ç?áÿªñt'?»Ã{¦zº?Üتß?»Ã{¦zºMIXED4FGL J1657.3-6232?èç"oL$WÀ(+{®ÍÀ:jª|?ìÀ;Ódύqm@^BT8fy@œ÷_GŽ4?Ê{mI.!?¶XYÞBÀð?êÂä`è">@•¤"^¥¿ïüÏ(ǟf?Ödü¿â	€²B¿æ™Y_ç¿éßv½Ì~É¿ë{j=‹|UNASNone?ïðdBG?bÛE}d?_Ñ7pÔ±L?bÛE}d?ïÛâæƒpý?<EüD¦Ñ?rŒªYŘ?<EüD¦Ñ?ï__o÷d?‹"C›¥-?"€?‹"C›¥-?ïÓQX¸'ú?^rê7Qµ?vWS¬+è?^rê7Qµ?ïˆÊ(`O?ŠÏԔwç?ø
rxPE?ŠÏԔwç?ïhT7î6ˆ?¦K\v'Ñ?'õxù¢)?¦K\v'Ñ?í}M´¤óü?£S`6aë÷?´'[FS ?£S`6aë÷?îŽp%×ß?—®šÂ‹H?§ÿÍ¢'?—®šÂ‹HAGN4FGL J1657.4-3917c?îÿ°­îv|@TÔ#&vÀ:_©³ÃÀ;ŽÚLè@Ç)_Iç€@±'!ûÓK?Ð
CàT"?á¡b§K3@	· QºÞ?úÖ=3'(·?ïùh6J>连à7|‡Ôº¿âYl¸K¿åßbцoñ¿æÃ^)+¿ïÞ´ -œñUNASNone3FGL J1656.9-3919c?í¥u—°Ž?µÛžq8µ%?²ÔSDܺ?µÛžq8µ%?ãǜÁc¯t?Ètüx®^ð?ØpÆ}8¡?Ètüx®^ð?ì^Ž´}Ã?¤I‹(+‡?½‹\è?¤I‹(+‡?è³ÜëEx?¥C³{Ld?Í0äRê"?¥C³{Ld?ç•ûív»?Ç`q´-ê?ÐÕô%‰?Ç`q´-ê?²¤/Ñ|_?¶Ç«äDÅ?í«z%Ðt?¶Ç«äDÅ?äÖ?O Nª?µ&»"!àG?ÖSa¿b¬?µ&»"!àG?ÉéfžÎ~?®.³–¡ÀÐ?酦XLzà?®.³–¡ÀÐ8MIXED4FGL J1657.7-4656c?ê¢
L™·À&"»À9$¯öÓ0"À:̨¡tYn@X=EZÓ
@ÿb›ÖŠ¼?Å3{''PÓ?ÀG/~ó¦?þÙ&ýšÊò?üÀ¤ ]Øù?ïß:Þ"_¦?ê÷Û8 Z~¿Ù™»þHoÛ¿çWšPx¾X¿ßÑÃ×/Ò¿ì*© öUNASNone3FGL J1657.6-4653?ï¬èQNú?"ýòÎX
?"Åë¬íу?"ýòÎX
?íEÏ[â?µ®Øôb
?³}чF°¾?µ®Øôb
?ì³»z®¶¦?¨€†…ج?ºb$*ŠJÐ?¨€†…ج?í&:áA<Ð?ÚjG±l?¶Î(ödÿ?ÚjG±l?êa½äv.?ÀFðKÏY?Æy¼n'G?ÀFðKÏY?äàµÑ¢c\?ÐûdÏ&]&?Ö>"\»9I?ÐûdÏ&]&?é!"cqe?´o%óy½?Ë{vr;öj?´o%óy½?ßÁç>p±¢?¿çÆ«Ôe?à`ǧ/?¿çÆ«Ôe MIXED4FGL J1657.7-4520¿ÑRPæ~¿øsÓ¼«šÀ9>0vÀP¾À:´ç]7@ \oço@ÿ¾¹ä'¼?Å9ügÅ?´»1CïÃó?ìr9¾g¯<@%e/.Á´?ï	Zò"Ý¿ëݟM7Á7¿Ív߇ϿçXࡕç]¿êÂìÿr;‡¿¸Ï¾Ä¡Z-UNASNone?ï5šÉ÷ì?¢'û\')?™L¦äÀ:l?¢'û\')?ï¾S&1†Ð?Žo\¶~e?€k6~?Žo\¶~e?ì—ñÌô?©›ó‰K¯?»@w1˜\
?©›ó‰K¯?Tl‹;?y%dx–?ÙêèLÍ<?y%dx–?êƒP!U*?Á‡çóø=r?Åò¿z©¿W?Á‡çóø=r?Àÿ†€?³+,ZL%?¥VãîOÊ?³+,ZL%?ëzc½Ù?°]}F˜8ó?Òžq›?°]}F˜8ó?ì ßLðãF?ªÕX·?ºù˜xåÎ?ªÕX·AGN4FGL J1658.3-4637c?ä͵ˆ–ÀDoÞµ,À9Zgä맃À:×qºWC@ Ÿê§Ê@‹˜AªÅ;?Çð½Ø=CW?»`õ
]¶"?÷­íCdٞ?ö¦+'Ëöä¿ïþ°nÈ5?ïþ`ù?Ÿ¿èýIúÑÿÛÄQ¾Ž›¿ëüº0ƒ¿áü\§ ÃZUNASNone?ï@Õfh.?£ ãÆ֗?—ÿ…S2úK?£ ãÆ֗?ìh`
?¿YÉä©Ò?¼¿S|ÿ¯ù?¿YÉä©Ò?ë†Oú¶Œf?¬	?-7ÿ?ÁæÀ%Îh?¬	?-7ÿ?ì–â㏇?¤ÁDàt?»OàèãƒÈ?¤ÁDàt?í>Œ$ñ?µò%žÎvk?¶ŸŽœ–?µò%žÎvk?ãH,'Ñf?Ôlô2túÜ?Ùo¦ú]Ý3?Ôlô2túÜ?ê—ëð°É?¯»%3æ?Å P=Á<Ý?¯»%3æ?×?¤ÈCG ?Áßs$‡@H?ä`-›Þ\0?Áßs$‡@H$MIXED4FGL J1658.5+4315?áè–Ž*@C#£ÂÀ;å§Ð"ªÀ<ý»9ýQÐ@!Ѐ2ë9Ê?ÿB0[è^#?Éq*º"º2¿¯ðZà:+º?à±&~
"@ßÀÅW†¿éeì"ÓiŸ¿ïî>ÅèW?ë	IàsÈ¥¿åMtýØÞ¿Ùd^—ºò?ʔG_ºû"UNASNone?ïýšyWH«?M¯ùe.?3,6/ìÓl?M¯ùe.?ïó}¡k?_8£O#?Yéá67ˆÑ?_8£O#?ïîƹ&@ ?^_ÞHˆwŽ?a9F¼â§à?^_ÞHˆwŽ?ï÷u	—Xw?A¦S@Gi?Qí?B'ô?A¦S@Gi?ïüX^Ìû,?=ÍwY=Ú?==	£%_9?=ÍwY=Ú?ïÏ9$ӍË?£ÖÔK'ï?xcm"yjŠ?£ÖÔK'ï?ï=œ?pjœßº?aG},¡?pjœßº?ïڛø¢Q?jUÎφ´?r²Ë#`?jUÎφ´AGN4FGL J1659.0-0140?Ø_ŸðL@7큾±À:»df²À;ÛVSÉ«°@6ÖS3XÈ?ý«m6d@?Ə¿P7{?Û¬D6¿@a¸¼-B?÷ÚJ><¦¤?ï ÊæB¿˜¿Ý ="(¿ÍÄüžÌ‰[¿à^ý':пïû½ü?ìôêÃùUNASNone3FGL J1659.0-0142?Õ2ˆÞ'?Êö>N¢Ù?åfš}¼·?Êö>N¢Ù?֞Yj]?̸N¡´×?ä°ÓJÑp²?̸N¡´×?à^à©´ªþ?µ<|¢Ô0?ßB>¬–ª?µ<|¢Ô0?ÞÞÌ1O	?´ˆ7Ł9?à™çXz|?´ˆ7Ł9?· ½°gJï?¹";©×ÝÖ?íèI¼â?¹";©×ÝÖ?¦KƒôÝ0I?¯¢o?î›GÀÍ©Û?¯¢o?¸¼öù˜ž!?©Ÿ]Ü\ÀS?ìèa èi?©Ÿ]Ü\ÀS?²ãɄ?£à8ÕؐÛ?í¼Ã†Á¿l?£à8ÕؐÛMIXED4FGL J1659.2-1443?î°¥¢™ûó@0ÉõœÏ®ÿÀ9úú0³&3À;ڻݑ@/@ô%ø¸
"@‹Ù½v?Ȉ}£–s?Ó^lÇÔ@} >ÏI@—†¡ð*J?ïýW¿.©Œ?ÐëÂßä¿äTŒÿØ<í¿Ùª‡Þ0Ly¿ï['\¼?åF>QÊMUNASNone?íÔtôž¢î?Æ2»ÃSëÿ?±\X[xÜ?Æ2»ÃSëÿ?ï$#ƒ#?¦ÝAÎVÖ?Û|–h1¤?¦ÝAÎVÖ?ìóØV¶—?£2…åüÆ?¸a=N}H?£2…åüÆ?î¤ÿ(óõ?ˆ–¾ˆ*J?¥°
m^¤¼?ˆ–¾ˆ*J?íR·Ÿý?¹ü±A%j?µjC	§å?¹ü±A%j?çRwœÐ?Сg/^Š?Ñõ[ÇÎ`?Сg/^Š?é2Õ·¤hø?°¾¬Ž€ñ3?Ë4©!n\!?°¾¬Ž€ñ3?è>Ø708?¶AhÜâ?ÏŸ#=¿ ?¶AhÜâAGN4FGL J1659.6+4918?ìém,B@CpޏlðÀ;§iϧr À<ßjT1°|@"yÅï@ÿÿ«Fj?ÓZ]āNÊ?¼.)‰_?æ×
˜n÷/@œ=D:¿íèØÁ¢¢,¿åP³a@➿àz=|bQ¿àœýÒ(V¿ßå»[5ZÖ¿ïý(_D´UNASNone?ïþûŠ¶Ž?#õ^–¼i?.pC†lKŠ?#õ^–¼i?ïóÀ¹ˆ€?[°"4h?XÒ,¹ð?[°"4h?ïòMÒñ©ü?a~‡GBó?[dZ@gø?a~‡GBó?ïøoߥ±D?5°5ÞMn™?N@€ &?5°5ÞMn™?ïýÍm±‰O?/åà™jm?1""ö¼µv?/åà™jm?ïз©
a?~O¶P#y?wö$#뫁?~O¶P#y?ïîÌÎ?lãc}ƒŠ?að3¶:?lãc}ƒŠ?ïÑ¥ëü+Ï?jÇMZFŠ?w-
 q?jÇMZFŠAGN4FGL J1700.0-0122?ç@h¼h6Ü@7ÝxqOÎÀ:oSשÀ;Ä76Íòg@Aº£@°'w"Œ?ԗg›ñ
?ãÁ1"·ºí@
çööl@ys×=>$?æA-ô/?ä˜`‰' ¿á…²œøŸ¿ë¥<e¿íÁ¼-BXj¿ïþ/EgéUNASNone?àN×ÃÃ08?͛Ų–§?ßbPxyŸ?͛Ų–§?ÓÆóBòÝ?ʆo…ÉØý?æ†^†ü'?ʆo…ÉØý?çÍõ¾?±Bg`dÙC?ÑþdöƒÍ?±Bg`dÙC?Ó:ªíH¯?°pøc‡"?æbª‰x[©?°pøc‡"?¹Vûf§q?¿©ÝÖ×µ?ìÕ "sdÒ?¿©ÝÖ×µ?­¶k¸:¤?ºîAUz?î$™DŠ¦?ºîAUz?ǯÊ!eš'?´ÊϬ#Œ?ê
w¦™v?´ÊϬ#Œ?'Óât¤?¾®Š´—?ïi`ïYÂ?¾®Š´—MIXED4FGL J1700.2-4237c¿Ü»­ù€'•¿É=4D«+À8N>X*cÀ9ñ²½W@–ë_µ@G`Æu?ǹNè›_?ÜnÛëMÁT@d öðŒÅ@ˆŒxô³q¿êâ‹`òË?ïüJ~Sm¿å-݈ܳ¿ì Ñ0à¿ïÂã>ÿ¿ïö'=¯¸ëUNASNone?䆚ËÆL?Ô¨Ã]NÞ?ÖòÊièsi?Ô¨Ã]NÞ?ÍÀև¿/3?ÅG‹Ë¶Þ_?èÊ^43?ÅG‹Ë¶Þ_?ÚNȯ¬‡?¶ýoÐõâ?â؛¨p)¼?¶ýoÐõâ?Óǫޞ9?²"gj|³u?æ*°ãs?²"gj|³u?ÌZÁù]z?ԛº€Äáq?èéO½¨¢?ԛº€Äáq?–Áé¹E?¢Ú•š*õ?ïI÷XͲ·?¢Ú•š*õ?´ã؜­­õ?¢c"uÍH?íc"ì…Ç!?¢c"uÍH?'…ç×[nU?uKg~›ê?ïµè`ÀÎ×?uKg~›ê,MIXED4FGL J1700.3-4557¿²(õ̯ÀyãìëÀ9&p­FÀ:ŠšÔ,<Ÿ@ÐÁ{µØê@#Ɔa®q?ʘÜñç?πåÇFü@c›{)Q@¶•bþ'
¿å‰¡iq³¢?ï†Nc:aü¿æüÚQοæjqáÕ¿ê4{'W]µ¿ïþêÁªYÛUNASNone?ì4p}Ÿ?Äo²úWŽK?¿7æ\|?Äo²úWŽK?í10׎FÕ?¹Dï`¯õ?¶vyAÕûY?¹Dï`¯õ?ç«n4Tà?´É£è«?Щ#—V?Ê?´É£è«?íyˆ=ëaÒ?›á–k8s"?´3¾/ò?›á–k8s"?åžbøXýÙ?ÉX‹´²,?ÔÃ:NM?ÉX‹´²,?ädä}ð?Ó«B3+P'?Öá67à ?Ó«B3+P'?Þÿ/J›Z?º.°0x²ˆ?àòhZ²S?º.°0x²ˆ?Øï‹fƒ <?Áiy'øv°?ãˆ:L¾/â?Áiy'øv°MIXED4FGL J1700.4-2746¿î%Ÿßtð@!¼—ú](ÐÀ:C	^M"1À;¸+`ÖÚm@N'·ވ@L'Iñ?Çݏ'¯›?°›»\âÙÿ?æ{—P=Ê?úQÕøÅy?¤; :XÓ?Øß-jä%¿ëàz©"¿ßþè(¿ãƒHõ<X¿àҍÖí·ÿUNASNone?ïøóüúÆ?OøAa}\û?Lñ0께›?OøAa}\û?ï^¾Ç{'?¡"¦V¬?"('·…?¡"¦V¬?hNô?‡×>ò'_?Ž">i[ß?‡×>ò'_?ïÐÿ¹`<?]h¬u_?w€|ˆ'î!?]h¬u_?ï¼fœ°ê?ˆMn–ã;6?€æX×å8?ˆMn–ã;6?ëeגÎyJ?Å{au:ê?Âh¡´Æ×?Å{au:ê?î6¬/Útf?¡0Ջ½Vñ?¬•=4 ˜?¡0Ջ½Vñ?íñ
ñҍ?ÛKa¬a?°s‡ŽKª?ÛKa¬aAGN4FGL J1700.8-5218¿ïG›qNæ‡Àßþó…õÀ9ØU)þKÀ;uÌ¥_ z@bQãÍo_@ãVg?ÏÚû#L`V?Ïud8#2@â˜E܃#@×;Ëz?ÖÊ¡¤U	r¿ë•X¢žÁ¿çn¿0,¶¿æùÄaÄ@6¿ïþùoÃz¿ÔÓ@h¥ÜUNASNone3FGL J1701.3-5216?ï¶AÝ£'?€Cx_îM?'xïzØ«?€Cx_îM?ﺣ2'M?¢Dýζ?È« šNQ?¢Dýζ?îÓI/7¿Ï?'‰´³Ì+Ú?¢Ëmφ?'‰´³Ì+Ú?ï<$ca¤5?y#S!Q<À?˜{s[Ýj?y#S!Q<À?î(ß^'?¦©Šˆ2?­~2£¸J?¦©Šˆ2?çÀEJÀv0?ËȦಐi?Ðuj ?ËȦಐi?äÆ•š«?¸ ^ª'U×?ÖsàÕöÊ«?¸ ^ª'U×?ç!_ÀHÉ·?´¬ÎÐi,?ѽ@nl'?´¬ÎÐi,AGN4FGL J1700.8-7304¿Äʍ֏pÀ2jázû]À:ÿȘŠ¥áÀ<w7ð1Uã@VÔ}›6@jÕ`ðà?ß{2{R[Â?à!ï^G3@vn¡žJÙ@[<'¦?ÜëÂFa
?æ÷©OBÇ¿à.Ìț¿çÐÉ{ßto¿åÕN±=û
¿ïæïÝ ,UNASNone?ïù× Qñ?S*Ä6Hl?H£}¬³™~?S*Ä6Hl?ïë–c=?j{#ò){ð?dài¤ÃË?j{#ò){ð?ï†Öf‡&-?'´åRê.?ŽJfod€¢?'´åRê.?ïÕ_¿¥"?Y‹@›¿¤F?usÐ$ü©Ö?Y‹@›¿¤F?ï÷²ZŸw™?VÐvß2:?P›Kǽâ?VÐvß2:?ï¹~éêêÅ?'}Gwå? EŽŒ@²?'}Gwå?ï6Š9ç?"€
»Ü7ï?™.¿?¢U¡?"€
»Ü7ï?ïCv²?"E2k<?—'<wqÓ?"E2k<AGN4FGL J1701.3-4924?á¾}9ø°À
2±-4À9Á.^¸<À;=¥."R:@JÀ¾ ·†@ Uûµ¤?ÏÊ,–?Ò,¬{ž†é@:ry\ã?þ<«tp–¿ïþÐW›È?ïý‡ŸñøU¿çÎÇ]øÛ¿å§û'Ü5ö¿ïþ'ö ?â²aFkõUNASNone3FGL J1701.1-4930?îê¯P1"?¨	:=øåÙ?¡U
ýµˆ?¨	:=øåÙ?éÜhSGó?Äz€,hÇG?ȏš^²à4?Äz€,hÇG?ìMƒI²6Û?¥•0CÊK?½"å²nI+?¥•0CÊK?ìR§•ßc?¤Â÷ÌT×É?½jÃWÙé?¤Â÷ÌT×É?ê96ýîü?À²ë lT?Ç$Gø?À²ë lT?Ñj<äp?Ы…o@)¼?çJá±qÈ?Ы…o@)¼?ÞúúPØNz?º"·
 rð?à''×"ØÃ?º"·
 rð?Ê쭝‡×?¹Œá‹†í?éDԘž
?¹Œá‹†íMIXED4FGL J1701.9-4625?Á"^¡‰¬À7´·,À9¨3ša?¶À:Ûd53¾s@/©Ì—Á@¥æ¼b~?Ðkj|uœd?àR=à
l@@
?:¬¤8@´™Æ»á¿ÖW}ë=P¿èÏ"Îš¿àôG/iz¿ê2þº…¢¿î?.Ö­ ¿ïSÅ¿½DÅUNASNone3FGL J1702.1-4623?å:Vu'Ž?ÌlHŽËF?ՋSúãá?ÌlHŽËF?ãVªB;í?Ïð
xäm?ÙRü«{ˆ%?Ïð
xäm?æ"_4‡µÛ?²¯$~y'•?Ó»A–ð"J?²¯$~y'•?å©ÉD#'Ï?´ƒËU"?Ô¬mw¸Úc?´ƒËU"?È+àîí³ø?Â<åvðTð?éõÄD"?Â<åvðTð?"¹šæƒ?ÈOä6ÿN2?ëZљ_?ÈOä6ÿN2?ϜRR?¶:1´Øå4?èÿzkxk?¶:1´Øå4?ªˆÐý¿ô? ¶‡ÿ^¾?îWrð.ô? ¶‡ÿ^¾MIXED4FGL J1702.0-3721¿æIeqca@+xÚq3À9¦Å¿'Q§À;vy!@ûÝÜ@MÅ2¥?ËbV6mzW?Ð ´«m×t@ZÆ3¡î@ZªBß"»?ï±ï,»J¿´{ƒ"…F¿Û»âï£ç¿ã´U'¿êS±Þ3ý^¿ðUNASNone?ïºåwF;?¢ÎñÄg°?(£O_j?¢ÎñÄg°?îükü'ƒR?¢ù°Øü? 9@:ôé?¢ù°Øü?íˆÜk×?¢<°1B–?³¹§ç¡K?¢<°1B–?ï
lq±±?H¹†aÂ?žRqÇ*'ó?H¹†aÂ?ép^Y҄G?ʵ±ÁóD?Ê>†˜µîå?ʵ±ÁóD?é\ú'p:Ù?ǑEM²³?ʌö?›?ǑEM²³?âUúw,?ºï"{ð?ÛT
ýÁ§?ºï"{ð?é=CàÞ?®åG¶Û›]?Ëãß
ð|ˆ?®åG¶Û›]AGN4FGL J1702.3-2525?êÍ®‰s@#à#éêÀ:9êØPÀ<Ğ*"@²Wz>ý?þý@´%?È`hàê*?ÒUûŸž@à•äÙ3
?ùàçß!ä?êý"à¤ðæ¿è¬ÍT¤?ÐCCrE˜¿ÙØŒ'Á¿å³I€C‡¿ðUNASNone3FGL J1702.1-2524?ïôgž~?]ìك#Ág?W1êÁÄ,?]ìك#Ág?ìå© •?¸«Ä« j4?¸×J·ÛºV?¸«Ä« j4?ï	È´Aï?'Ô·â5èæ?žÆév
O8?'Ô·â5èæ?ítý8XÆ?•^J…¬
?´X=?aÑ?•^J…¬
?ïøNÚî[?fº']F‡?Nė áï&?fº']F‡?áÓÜØLv•?ѐ-{•~?ÜXFOgÖ?ѐ-{•~?ì¸ÞQô-S?¦¾Ï± Â?º9
p^•j?¦¾Ï± Â?å·äFÕÁ,?·óŸ}?Ԑ7rT}¨?·óŸ}AGN4FGL J1702.5-4803?ïO±"®RÀÅS[ǦóÀ9»[>À:曶ªK™@¸HýÏ@Á`Dä5Ÿ?Ý©Ga"mÛ?ǒ&>?÷1Me
 Ò?ûæ6mÐ=¿íöÞï@5?ïõuüŸ¿ê¿Õ£5#οéJ>xᓿå¦ÿéYËM¿ê¶iLUNASNone?ïo8l­þ+?®‹<߄_v?'òog¤¦?®‹<߄_v?í#žÅá ?»(Íû1Ja?¶ã˜)?»(Íû1Ja?슅9»7¤?¦ñwØÒà$?»«Ö2&Bà?¦ñwØÒà$?î%ö?˜"Ð]Ï3Ç?­¯ "Ÿ3Ö?˜"Ð]Ï3Ç?éƒÁ-åÉü?ÊWïy¹Ä ?ÉðûHhØ?ÊWïy¹Ä ?â²ÕÕ+o?Õr0Á`T?ښTU¨å"?Õr0Á`T?çQICôT.?²ÜaP *¢?Ñ]mxW¤?²ÜaP *¢?×ôód°Ñ?ÃÒÉNp®ò?ä†~M§—?ÃÒÉNp®òMIXED4FGL J1702.7-5655?ê(Ï|ªuŠÀ"u?À	oëÀ8BÃEdŽÀ;EeìÃã@{¯xÓü@ÖÔ=–?¤¶Pð?Òò1ÀíE"@'ÞSó@/;Ÿheš?ïÌ
ÑyÛ¿Øm-_´›~¿å\iànj¿è¨ujhS¿í†ý )Uº¿åxYã¡$¨UNASNone3FGL J1702.8-5656?°NJ«hܵ?¶¯6<f³?íö6ª®aI?¶¯6<f³?½tÄ".S%?»)øPM??ìQg{º5›?»)øPM??ÈVV1ÿ›E?¯®E"I$?éêjs€/?¯®E"I$?–T+öŽ¯?‰Ãùiã-?ïM^£W;?‰Ãùiã-?½ºÊ/¨S
?ÒL›[ˆ?ìH¦º
õŸ?ÒL›[ˆ?›õFò
|Ž?§À:Ž¹o7?ï UÈ´dK?§À:Ž¹o7?À[£´ûtÖ?ªßˆ³±[?ëéÁ"Ë?ªßˆ³±[?`½¾yJõ?W¸šM?ïÿúS1š?W¸šMPSR4FGL J1703.6-2850¿ïê*
D·@¨E/‡­À:@€#À<8¸®1×@ Àåä@Ó~9Á®?ôæç€,`?؟ND0±y@=®ˆ*Ü@o¬.œ Š¿ï"ôÁ?ïU"âOÀÞ¿ÒU,«¶¨¿åÜ_ag¿ì´¡mM‹¿ïÿû-2h2UNASNone3FGL J1703.6-2850?ì±xX
i?µªÅz˜Ùr?ºt?å?¬¶?µªÅz˜Ùr?ë¢Hkm{?Àöüm›±C?ÁvÞRJŽ?Àöüm›±C?å_¯ºÏÊ?´®²S¦{?Õ@¡öŠ`l?´®²S¦{?îD­Ö´Ïw?SSÜmv?«µ"—F½†?SSÜmv?ä°«OñÒ?Î^"ð&2?֟ة`\?Î^"ð&2?Ýĵ!Õh?ÑI÷ë^ˆL?á¥tïL?ÑI÷ë^ˆL?ÑèúO'ã˜?·Î	<ü?ç'Ø74?·Î	<ü?äøÎÑðß7?·œy•9¯ñ?Öb\A'?·œy•9¯ñMIXED4FGL J1704.8-4030?ïŒßÅß?Û@¬B"£`À8yÓ3[AÀ:LèÁõÙ6@Kû+/@äÍt'y?»¸€®­?Ôñ[!ŽÆ@Œ[J©q~@y2 ?ï֘Þ2и¿Ì,gç𿛿φ\¥óD0¿ä³¼ZŽÂ¿éÚQÎ_¿ïÿÿ" 5•UNASNone?ª4{æ[?½z#˜Çž?î\¸NX¿?½z#˜Çž?Ñ"¸ìñ?Æf"³"?çn£‰‡}¸?Æf"³"?ÐÆ 'Ó-º?²$^ŒÂ‡?眯ìi#?²$^ŒÂ‡?܄ùpçE?¶*±KÀ\w?ὃGŒu^?¶*±KÀ\w?º[pÃPf?ÐíJò¨º°?촑ç•ó>?ÐíJò¨º°?˜ÈGóWÒ¯?¤é+E[²a?ï9½À.G«?¤é+E[²a?±'][µ?ªšh2¯¯Ï?íÛTº†=?ªšh2¯¯Ï?ž8Ïߎ¶á?ŽËÝIØÍG?ï9€Ì‰?ŽËÝIØÍGPSR4FGL J1704.9-4303¿Ñ"Ý ÷S¿ò'U^×%ìÀ9a@®Eù	À:‰q€Ø@ %ù	@Æo@SjZç­#?Õ¥dd®€?꺪ùš‹@2&ù'Ô@í‡@¬n?ïÊ4f?êVžrFny¿ÙÇU¿z(æ¿âuÂú»ó¿îÒ¾©HŽ¿ï¸fC*÷ûUNASNone?æ'ÿã¡6?щÎr5ÉÞ?ÒÜ8½"?щÎr5ÉÞ?ìً
ÝË?ÀÏBÜ&9®?¹3§'ϧ¨?ÀÏBÜ&9®?ãîٞ†,?³†É×¾²?Ø#ÄLÂó§?³†É×¾²?èjæ¹ï
Ë?³O"ܐ?ÎTeCÔÒ?³O"ܐ?Þp¾a­£?Ï8¾º‡È-?àöÇ Ï)/?Ï8¾º‡È-?èÐk,É·š?ÍtJÂ=t!?̾SLÙ!š?ÍtJÂ=t!?âK}
êÞ?µZröVXÞ?Ûiä+ÊD?µZröVXÞ?Ødn?×9?¿æåI¹?ãÍ÷Èàc?¿æåI¹MIXED4FGL J1705.1-4748?éJ¼‡@À+†±_ˆýÀ9«8bGÀ:ä€üê¡Ê@C"~øX—@+ôË—¦?ÔÏ ´?ØôóT¡@ß	ß3Ø@õkšWÛ?ï{úýŒ³,¿æêÛuÜûï¿äXŸ›fM¿élá8"œ¿åÆ×õõ»¿ïÿÚ
¢ñ1UNASNone?íãâw¦L'?ºÇ^ÇíY?°àìC©…Ç?ºÇ^ÇíY?ì"Ý'ç=?»,›‡
.?»ÙãhÆ?»,›‡
.?êTH撊u?°žéEƌ+?Æ®ÜeµÖ*?°žéEƌ+?íLpZþJÁ?œíÞT™?µœ}&ÃÏ}?œíÞT™?éAž"ïÕ?ÉÕ¸ÌÃEB?Êù…¬@ª?ÉÕ¸ÌÃEB?Ü=ªñìÓ?Ó[‡QåÈ>?áá*‡	–y?Ó[‡QåÈ>?ãì-=ƒvË?»unZëLÙ?Ø'¥"ùj?»unZëLÙ?ÒËÈPc¥?Àò"܊?æš×÷Î-?Àò"܊MIXED4FGL J1705.2-3850?'þµä™k?õÌ߬£a™À:
E®_ú<À;Ë°Àý‹±@Qlut c?þ(j'TÙ?ÑYF'ÆCq?êøPV×@0šú©]@3D™âê›?îÊâa‰‡Ô¿ÏSJ˜Õy¿ÒZ-òï¡¿ß9çíºƒ¿ïó£¼2?舘TõûšUNASNone?íZ{ìé?»Ú\Ÿ×æ?µ/œ"P†?»Ú\Ÿ×æ?ëîG³ó·ó?ÀËq@g¬À?ÀFá01 3?ÀËq@g¬À?郊š^v¿?¬ºSfnî?ÉñՖ†%?¬ºSfnî?êÌJ"Ìûò?«E"j/Ê?ÄÎÕ°Ì9?«E"j/Ê?ä>]‰P©Ä?Ëg;B	²?׃Dí^¬x?Ëg;B	²?Õ¹]Ñõß?Ï~o¯îÎ2?å#1Q?Ï~o¯îÎ2?ޔ3Xœú!?·@ìÞ÷1?àµæS±'ï?·@ìÞ÷1?ÛnAÿ S?½S®d4q?âHßoÖA?½S®d4qMIXED4FGL J1705.4-4850?ïÀ¨M€U?ÀÌ}´'mÀ:9V"tnÀ;‹«‹3¥I@8‰ëPÆl@S|~֟´?ÖœÈù¶?æ‡ÁÕÍÒ@ìMìm@8JŸo?å',Rnaݿ∉ÁµA–¿Ú͈ßb%º¿é¹ëžŸÿ¿ð?ïÿÿÊPËUNASNone?êÿDî
xï?ÅÅÀuã?ÄìGÖF?ÅÅÀuã?ìԖãºW³?¼Â£þøC?¹[HáQ[k?¼Â£þøC?çŒf†­êÆ?¯…»­u¤?Ðç2ò¤*u?¯…»­u¤?î[œþþÎ'?"æy'^$à?ªF0ǚš?"æy'^$à?âÃ끿|?Ñ %	#ë?Úx(ýò	?Ñ %	#ë?Òïa*?ÏË3÷˜?æˆOwêûÀ?ÏË3÷˜?׌7€õ³Ì?¶ü¼üDZ?ä9ä?…&?¶ü¼üDZ?à0qj"?À­çhsJ¿?ßõŸ*÷ê?À­çhsJ¿MIXED4FGL J1705.5+2907?ç9Ÿõíò%@AR¤~Ïé¸À:¿5ÜZßJÀ<\m.׃à@ùpâ†@Ðfd¸ç=?Ȓõ%0'?¶V¯d1,ô?èäK8ãv\?þŒ³t·?Ùiå‡ó¿ßsd%Ä`¿êA_f¿ç	OŸz"+¿îìSE!rA¿ïì`Eºõ4UNASNone?ïâeËêWU?oJmíh?mš4È3!?oJmíh?ï¨dlÞr?'¨s´Í?…æäÒ²Qè?'¨s´Í?ïql¥M`?‡‰ôÿԈ™?'Ðf.ê?‡‰ôÿԈ™?ï:­Ìá<?}ríñÕ+Ö?˜ªOÿ" ‡?}ríñÕ+Ö?ïw¦Õ—?žÇN°©'?œ]±F ?žÇN°©'?îd÷.±T‡?²Á¿N‹´?©°ƞ‡?²Á¿N‹´?îàïí@é2?—‡\ýTX?¡ñ)]·å?—‡\ýTX?ê[¬³Ÿ º?«_?¨!ø?ƑM1ƒ}?«_?¨!øAGN4FGL J1706.2-4950?å0[ÆÀžÇ†;îÄÀ:ðp@üÀ;ƒ€ýÁa_@§l®)±@‡ãúû÷?ЯIĚ#W?ÞúôþD>@e‰ýDcÝ?ø
t";¿¿å\·ûeg¿ÖóI¨Pí¿ã¾V<"¿ëä ©m¿î÷Æ`!'î?ÞFžJ''UNASNone?ífæñç
–?ȟ܉ƒKú?´ÈÈo}¸Ô?ȟ܉ƒKú?åæ¹Öâ
³?ÌqѼÔ9Ü?Ô2ŒR;êš?ÌqѼÔ9Ü?ë`k2(R?¥¦?ÜÄ?Â~S7_'¸?¥¦?ÜÄ?êâ9èÑ\¡?¨ÙXu‡Í‡?Äw\º|?¨ÙXu‡Í‡?çL,¿â¿¹?Äv{ K"Á?Ñg¦€:€?Äv{ K"Á?½*‰ÒgB?Åcç:Ž`?ìZ®Å®S?Åcç:Ž`?ÙaåüQRa?ºG_?ãO
×VÐ?ºG_?ÁìبD¥?±fÄ(Ó!¿?ëºDÉÕî×?±fÄ(Ó!¿MIXED4FGL J1706.4-4609¿àÂk»oáÀ	ÄȼœÓáÀ9¬¡´NÀ:ÜC8cõ@ !¾‡z]@åàdYEì?ÜnÖwpyæ?ÖÝqà˜Æ?ýƒ3ü†Ï?þ±ì<É¿ïô‡'YY8?ïú:þпׅì~à¿äW¬ŸZή¿ê¥cÒ7oÙ¿ÕW`NjUNASNone?ë킴r/j?ÅÁâ"pv?ÀIõ.7BY?ÅÁâ"pv?ìð:ªmHÐ?¼·†r(?¸~*ªÝë?¼·†r(?çðŽ½}{?²D¢˜Ý?Ðâ…é	?²D¢˜Ý?ìs"€Oñ…?¤ˆSëÍ^'?¼ccý€sÙ?¤ˆSëÍ^'?؍±|lë™?Ï0gÉ4^N?ã¹'AɊ3?Ï0gÉ4^N?ãà}Àígï?Ԕ—äZ)?Ø?~%0!?Ԕ—äZ)?Þç:õ|÷Ö?¹4¡ëtC#?àŒb…A"?¹4¡ëtC#?Óêê»[q|?¿ç ¯ÅL?æ
Š¢RGB?¿ç ¯ÅLMIXED4FGL J1706.4-4649c¿'›ãý"5šÀüœü$©-À9Ëû¹IÀ:ôÞW(Ü@=GöŽ½@^ú|2€†?Ö÷Ö»¸þ9?íý«w@	ízÂ=ý'?ÿ¦Tè凿ïÿ¿h`;ª?ïý­àx{<¿éðˆ=ќÀ¿ìZ¬‰`fr¿ì…;=ð?ÊÊ¢{žHUNASNone?éÕßÖóR?˝1$vh"?Ȩ€§°2¸?˝1$vh"?ã®äÇ«?Î}
°uš?Ø£Ì7üp©?Î}
°uš?è€Yaù¢Ì?¯CÒ1£ž?ÍþšxtÏ?¯CÒ1£ž?äYr¦Õ[+?·,ßÞ¬±?×M²UI«?·,ßÞ¬±?å]džg?҈¿_YŠi?ÕÛïDpó2?҈¿_YŠi?¿Î'Ö2Ò?ƺ"'°Ó-?ì;9¥¾?ƺ"'°Ó-?ÝPÍ´¡?·<P?íݒ?áW™%ø¯v?·<P?íݒ?¥Q¼aòÂ?›øºøu-?îªä9ûÏD?›øºøu-1MIXED4FGL J1706.5-4023c?잏8ÜYL?͒Fiö¦À8…™1"ÎÀ:g°éAx@Xô"&@qœûMê?Ɂ©ù8:¯?ďHy]d@o¿@OÂ@*5³–?ïýFA­¿È+³1fª¿æÅ»Áã¿è(žŸ'×Þ¿ë\½جտïÿúÁҝÇUNASNone?é_'1Zñ?ÏIÉD#"?ʁ»:—ð;?ÏIÉD#"?îf7Z<ë?¯FŠ´ì‰À?©Ÿœ‹8O?¯FŠ´ì‰À?ã$¥Ñ¶@™?·,ƒ6mß³?Ù¶´\"~Í?·,ƒ6mß³?î?Cñ¶*
?"¤
òÏk?¬Àá-Ã7?"¤
òÏk?æ\é¨$̾?ÏD°Ÿ3{?ÓF,¯¶f"?ÏD°Ÿ3{?è+/¡¶Ò?Íéɒ…©"?ÏSAy$·£?Íéɒ…©"?ââM^úٝ?µ®TßdÛË?Ú;eB
LÆ?µ®TßdÛË?á"sÐ1[B?¾Ó}^-:~?ÜÙ_I|?¾Ó}^-:~8AGN4FGL J1706.7-5525?â±d0×
mÀ!"½8SLÀ:-únƇÀ;¯2c)›@ÿwšôŽ@°\‰mÒk?îŽ|?@²£?àµë÷öF@î¯?ôÖ@^Ѭ°w­?éՌŸ
FÖ¿äÜ¥R4€:¿ëM£Œa¢²¿è!ìÿ.¥¿ÛBwî¨j¿Öº
›5¦UNASNone?ï`à€ø?§ÈÚ…jÍ?"ãð(fx?§ÈÚ…jÍ?îÌ3÷Ë t?ª
!v~T?£<ÀÖ\À?ª
!v~T?íPÜ#Vò*?¤yK"³§?µyæ'I-?¤yK"³§?ïfl0)é]?€ªæSˆ-?"2yúÂÔP?€ªæSˆ-?ëÄTÝõ5™?Ï5F°Ç?À+)œ?Ï5F°Ç?ä3YÜjN¨?Òÿn"96?יLG+b¯?Òÿn"96?æN(y½9?»nkSÇ8Ÿ?Óc¯×…Ž?»nkSÇ8Ÿ?䑍a`²?Æ$}[[­?ÖÜåá=>œ?Æ$}[[­AGN4FGL J1706.8-4540¿ê¤B€ÆÀðîÐ,ӞÀ9
:¥"À:x3⅛¶@Òå°@Äú¦#ë˜?Êꡞ÷?ÍWåÐD&@q£EêÅÜ@5,ìG;~?>t3¿è 'w"Œ¿è<yÎ"7b¿ëZÉD'¿äÃ4½ÌÔ¯¿è
q=Yý¢UNASNone?èetkP?Ðî^†·Ùd?Îj.Sò½Å?Ðî^†·Ùd?î•'G?®›þü?¦¯æ곧2?®›þü?è›aÕT}'?²¬•è½¡¿?͒xª®c?²¬•è½¡¿?î‰ ™ÂM1?'1Ò¦y¨˜?§möb#^õ?'1Ò¦y¨˜?ëj©T€=†?Ãº´­'k?ÂUZ­ÿ	é?Ãº´­'k?ç˜8gG?Ñڃè
™?ÑÐÏǏ1r?Ñڃè
™?æ­uæÙ_Ð?µZ"Ïýr¡?Ò¥2M@a?µZ"Ïýr¡?Þ0.%}?ÃcžÇ2>?àçè·íuA?ÃcžÇ2>MIXED4FGL J1706.8+1319¿á®wEB«@=
ù½Æ À::¼µ'•À;ó
÷9ˆ@tŠ‡¿@˒}E¥ü?ÁnÝÃÀÄ?³jzF?À»~ãH@EÝ
$q¿ä#gC8N¿ä>Yl'à¿ì›Cót×B¿èÈΪŸ¿êb!LÖÈ¿ïðCÊZ+ÆUNASNone?ïâá¦p'?"K~šðõ·?mYs¸¿?"K~šðõ·?ïãw{.?~pÍ©àÉb?lüˆI¸¢H?~pÍ©àÉb?ï%*/˜8?•ÌWt²º?›_³-Á?•ÌWt²º?ïíáñæÑu?Näm'ª?bð»…?Näm'ª?ï["mW=Ì?›'£	&g?"rUF"?›'£	&g?ï…I裺Q?—¦t,ÿeÇ?Ž­…á`?¡?—¦t,ÿeÇ?Ñîí?Ÿ›ÛW?§gòá0?Ÿ›ÛW?ïX.[ÌÉ6?…±¹¤e O?"ú4?oQ?…±¹¤e OAGN4FGL J1707.6-5351¿å<–¨ðÆôÀßþmXÈïÀ:dT§!A™À;ÁåN£Ò@—›±vÚþ@œ zûI?ƀ"9»¸}?ŠéÖë+)?ÈæX%?èhkêòÃ?ï´Ó³¬j¿ãSæ1!àû¿ê.‹-Æ¿ä㮀†x*¿àÒ1@ìF¿Ü¥Ûüëx‰UNASNone?ïöa¿\¼?Qƒ7…ìS?S<Ò†×Á?Qƒ7…ìS??©|ºŠ±È…?œÿ?vôE?©|ºŠ±È…?ïŸÁpù?ƒ™¥ygó?ˆ?Ï R¦?ƒ™¥ygó?ï^3Uܚ?u_
+§Ö?9Ûr­?u_
+§Ö?ï³Â.…›Ø?ˆG'-ð?ƒtT¢,?ˆG'-ð?êt|Ý(î?Ɏ
|':N?Çú.‹\H?Ɏ
|':N?ï	¡Å?ÃB?"¼<ô·~Z?žËÇ[w3¹?"¼<ô·~Z?êÂÔ¦_ü?²ô´j§Ôö?ÇÜô­f€?²ô´j§ÔöAGN4FGL J1708.2+5519¿²ˆãÙå¬E@BE"V!uÀ:ò¼~ ïÏÀ<‰
ä¹S@4,AQ"@ÁÛsX½?Á~$É
$¬¿²¿^z3͸?ðÞu†"Ú@•^XûIJ?ìñeh9¥=¿êŽÆÚ
M¿éóëÇkd¿â³@S'D¿ïÿï¤h)µ?ïÿyYˆUNASNone?ïð¹Û¥Ð?cU¦×0?^ŒHKëà<?cU¦×0?ïî³OßL'?dÆ:¶±Ë?aL°:Ðuv?dÆ:¶±Ë?ïÆNÌÊQ?|Ö¯êGî?|ýØ¡Ùçb?|Ö¯êGî?ïênÚÒ?Ss"½÷?eà'X%þ?Ss"½÷?ïâ˘*"å?têÅ^s?m4gي¢¿?têÅ^s?ɠÿ?–.Ü›?‹–"‹dc?–.Ü›?ïʥׯB½?*Ÿì›Ù?z­±5ž?*Ÿì›Ù?îÏÇÙÑu²?•¼ª{û4O?£'a0Öé?•¼ª{û4OAGN4FGL J1708.8-0923?ë0rÛâ@1Îû"‰µÀ9éÓbCÏÀ;tgVPn­@¨¯Ýþ£_@Æç£è`?ÏêéWòÛ)?ÎÀ|œÞ…@úälü'?ý¢™gŌ?ï;š«'"?ë†'_8u¿æ3ý}Ħä¿è:¥Ž¦¿ïü‰Þ™–¿ïÿþBe«+UNASNone3FGL J1709.4-0917?îQ¸þÓsõ?¨ïIZ"3?ªäpÈÀµ?¨ïIZ"3?ᒾç+??Ìò+Ò§éO?Üڂä1©?Ìò+Ò§éO?ìÎEú¤æ?£M¨b0âü?¹Ð,@?£M¨b0âü?ä/°JÀ)?±ä£Mw'?× ŸËj®?±ä£Mw'?ãËãéÒtµ?Ǻ?ÎÄk!?Øh8,[–?Ǻ?ÎÄk!?ÀÒí!mc?ÆÄ[Ÿ¸?ëËD¿w¤§?ÆÄ[Ÿ¸?ß#;@?W¦?¹C'w9±ø?ànb_àT-?¹C'w9±ø?Á³Â²1?¯Ð¸:¾ã?ë"\|4?¯Ð¸:¾ãMIXED4FGL J1709.4-2127¿ÇZ\Þ¹o‰@%ãU>S"À;8ÿI÷š×À<ǂ4"F|@ ÝɅ¯Ô?ûT^[Õé¬?׆ncàÐ?ïò%ÀoF@ُ>Õ(?üïTa+>¿ï2QÁ"³§?ïýµ7"Ñ‹¿Ørê"ž ?Úu^<¿íAWîÔ^'¿ïýÜÚa
UNASNone?åÉF˜ÉB²?ÎÁ
Ï©ÿv?ÔmrÎmzœ?ÎÁ
Ï©ÿv?Öí7"c?Î¥JÁ‰¤?äü	d=þO?Î¥JÁ‰¤?åœÔeX°?²ŠÑòfêd?ÔÆW5Nžý?²ŠÑòfêd?×ÕúÎ<äb?¶ß=SÍ}?ä˜áÏ?¶ß=SÍ}?ã¬DX8j?Ò&©Yw?اwO+Ï?Ò&©Yw?±*Ç–?ÀüO=Í7x?íÚ½Ì]?ÀüO=Í7x?Þ'©Ïán?»)9p?àÿ7+I?»)9p?¶Ks帩?°J
ÔqK?í?–'Z
›?°J
ÔqKMIXED4FGL J1709.4-0328?ļ\Û±}@4ÅE¥ü~kÀ9hAK#êÁÀ;µ´+W€@˜XpÚ^@ORƒZ'ô?ºÛÅc!?¼…ùԗÇ\@tt–ªÑÐ@ÌûÎÂñ,?ïʑô‰ª8¿æÃ:aû›¿ä	z!Úh¿æFÔ©¿êIßÇü.¿ïÿ (ÿӊUNASNone3FGL J1709.5-0335?晴•eϵ?" BÍ|l…?…ÛZœ=>Î?" BÍ|l…?îBu°Ü+e?®¸SÂ?˜+?«Ø¤ð…{º?®¸SÂ?˜+?î×,øµ¢?–¡÷×lÖ?¢0€€Œæ?–¡÷×lÖ?ìï[é=y?›¾OƒgÜ?¸‡
l9·?›¾OƒgÜ?ë"²²¢Þ?µá©éøö"?Ãí­55tŠ?µá©éøö"?æ~ãòr¯?΄¡û<÷­?Ó8Ü¢?΄¡û<÷­?ëlÞ^*éÊ?­B\¹÷?ÂL†‡TXÙ?­B\¹÷?â£w4â?µ¶NqKÏ?Ûιó–<?µ¶NqKÏAGN4FGL J1709.9-0900?ïíiÑfÖ@1ÆüvÀ9þCiâÀ;­iQ;@z*¨J6…@Æpº}>ð?Êpkø̄þ?âžÏ™/çN@œ4;pïV@ìÞDïHM?ïö8 WäC¿â @|ÇÑ»¿âºJÿ'¬˜¿éUao0º¿î×nF.¸z¿ïÿýç!éUNASNone?ä¤gRkÿû?ÍéAËZ?Ö·1[(
?ÍéAËZ?Ï#h²=vÐ?ÆÖ ?‡÷¨?è7%Óp¢L?ÆÖ ?‡÷¨?â«e_²º?³'»R•½Ü?Ú©5õ@š‹?³'»R•½Ü?×1»Ÿ‡?±jV>ˆÎ\?ä{ç"t°<?±jV>ˆÎ\?·^ï"@÷é?¼'͈ŝ?í"
"]ã?¼'͈ŝ?ŸÏ‰09Ž?®—KýØ©?‹öK?®—KýØ©?ÏRÂáwºÞ?²0Üë`³4?è+OG¢I?²0Üë`³4?""¬=îʏ?R½ä[?ï[ZõÌ?R½ä[MIXED4FGL J1710.0+4629¿ïínýR•h@B/Øf€À;	|gY«mÀ<¿¹üæp@±Æáü4?ü=''N#z?׬9¯N?ÚÚÙjj&@?mƒ'˜?÷Ï'EZ?¿C¬ÁÙB–¿è¸V¿×-۝ôr¿Ý"§BÔ¿èY`Y+"¿ïø"PŒàNUNASNone3FGL J1709.9+4624?ï©1uN¥?®}±
îSW?…³¾°jƑ?®}±
îSW?î#(`hÂÙ?¯ö֊Ý?­Íy÷¼k?¯ö֊Ý?ï;KüU?:Ëdæ?˜–þ½'š?:Ëdæ?ì{|¶gŽ7?—㯍,ëõ?¼$LÎF?—㯍,ëõ?ïIß]¯Cá?™ã|Òé?–ÄDðå?™ã|Òé?æcÆute?Ìg-¶œ‰¹?Ó8s÷6?Ìg-¶œ‰¹?î.Ò~E3? ö[ñ«D
?­òÔ¬Ö? ö[ñ«D
?â¡Õk	–à?³ _d
5?Ú¼U)ìÒ@?³ _d
5AGN4FGL J1710.1-4541¿îöÏsù«À·'Ôà˜À9Òí˜oWÀ:Ä]ºÆ:@ ÝÒÕzp_@­D¦">?ÅáÈÇÚt«¿öå=öŸ?ß$¥Ñ¶A?ûǕ*t¿èI ]?é|×V"ŠŒ¿µIÖã§å¿é=êFZWd¿å<jIIõí¿Û+Í
dl'UNASNone?ï¼&ɏÍà?Ÿ†Å;ó?€öM"Íwü?Ÿ†Å;ó?N³?™²I h'?‹¾ú®?™²I h'?칸"°N?¨•|µzy?º2;ÚEŽ?¨•|µzy?Œ‡Ét?z¡q°?Œž\äìÛ?z¡q°?îTÎ}?á?§ÕHáåž?§*³›ó?§ÕHáåž?íiµÄP/ ?Áp
²"?´²QߤH}?Áp
²"?ìR|åŒiä?­ÈZe:è?½lӜ°á?­ÈZe:è?ëÊwÇÚ?²!"ßÇÞù?Àז à—§?²!"ßÇÞùAGN4FGL J1710.3-3039¿èÛ£•NŽâ@¯¸á]}ŠÀ9íŒa¢²GÀ;"\sž]N@Ž`¹~;o@Ž8¿,Ñ?Î=ÄfKä?Õ]mÄS¬z@˜:ôȔ@0…·e¿·òÅYç?å«ö"o³í?…§	Þiñû¿á¸FB"‰è¿é¶É™"{¿ïò…Ãù¿tUNASNone?ï3±óB"?›
g¹¬ò?™‰ÝF¿ˆ?›
g¹¬ò?ìÌ/Ãç÷?¹·îvô0Ç?¿ÙžàÀJ?¹·îvô0Ç?ì"­+L?£¹M×ë?»g▧e¤?£¹M×ë?ìYzÑh¤?œÛPVS?½4)tºß\?œÛPVS?éK½Ud?Á¬,Zô9Æ?ÊÑ
«÷âr?Á¬,Zô9Æ?à­íʯwc?Ðk·:¶¬œ?Þ¤$j¡;?Ðk·:¶¬œ?ââOâý?¹"l—ËÊ?ÛÚ;aø:?¹"l—ËÊ?ß«^~¡¬Ê?¸	Æõ"¹'?à*PÀ¯)›?¸	Æõ"¹'MIXED4FGL J1710.8+1135?åý(8·	@;‡dº"¼À:²?d™ÝŒÀ<*.wÐ@p›ž‹@}ãZ­Ë?Ù´…-Pñ?ïÿþˆ0»Š@¾¼@ŽÉ@ÇÀv?ïíöé	:¿Üè@Ü;Ç¿îÓä¿ïÿÀ¿ù)Í?ïûJî:Ü¿ïþ@ý÷DUNASNone?ïv"TRŠ?¬‡æv"›ƒ?'-•~EÄõ?¬‡æv"›ƒ?X«è§?·P"aò)?¥TZs‰§™?·P"aò)?었Þ>ð?¦×Ø£v?»C¹H"?¦×Ø£v?ïâÑf@?l°˜KTSø?m.îwcÜ?l°˜KTSø?îݶéê?°;[œÝª?¢$ž–X?°;[œÝª?ãIf2C?Õ^Uå~Ž?Ùm3Ýۛz?Õ^Uå~Ž?ë&'Jái?¬BÃþ³T?ÃgbÔzYý?¬BÃþ³T?ìCHK1«?À'ÀõdVÓ?½å½§žr¥?À'ÀõdVÓAGN4FGL J1711.0-3002¿ïÜٕ©@'Õü3ÃÀ9ç…w£¥ŒÀ<ìxc¾ì@äQ&@áf?È9ÜÛÖ}?ï@r¶ÖÁ@Å?9ѳ?ðSœà ?ïÿÿ)@k*¿â pÎI¿Ñœž|ƒ8¿êYÇòrxÿïü"Åý¥³¿ïÛÖ¿•UNASNone?À'èpþV?Ñeg®~?ëۅãÀjz?Ñeg®~?´—еWÖ?±Çõt!??ímégÑå?±Çõt!??·Êbþþ?¯œwuO?è^
gz@A?¯œwuO?r³D"?\Ó;{'%?ïڙкÜÏ?\Ó;{'%?»_ɘ~«F?Î}'+5?ì"Ìð*—?Î}'+5?"êÈR@?‡úì3­G?ï¯ó°'W×?‡úì3­G?º]B%iq?¥ù)#Ê;v?ì´W»RÑß?¥ù)#Ê;v?t­+°?	…b2H"?ïÿd[–¡?	…b2H"PSR4FGL J1711.4-2526?ꢖ.oË@ ‹ææS†À9¾çBsBÀ;€¨AÓ	'@ž†¦!è2@©õ1?ȇiÁ9Æ ?Ìmš7NJç@MNûÖ7@ºJyJï'?ïì2ðî¿é¨/"BAÄ¿ã%DȆìï¿çÝî'ð2-¿ïÿ÷fÔJp?ïÿ!ž5_³UNASNone?ï°þ*÷N?‰Öª­Nh?ƒÀuq3Xy?‰Öª­Nh?îåµy$?­5ìo¶d?¡®"§'6Á?­5ìo¶d?íð?ÝTs9?œ¢¨¿"îD?°~¤˜=?œ¢¨¿"îD?I
?w;kh&©?Ž;êMM?w;kh&©?îMzØÊm2?²¾ÿêzj|?«(Roéá?²¾ÿêzj|?濛({½?ϲHX­·?Ҁɯó‡?ϲHX­·?ä|[o´»+?ºz…Æí©€?×I –‰«?ºz…Æí©€?êýÿ¤‡Ö›?±_©lån?Äm॔?±_©lånAGN4FGL J1711.9-1922¿èsf*Æ@'PoiDg8À:]^ˆK"|À<eˆEßÞ@g¥3€µó?þÆxõ?Æ6Ükü(?à{:Ôd¬@Ê~=ó?ütá0‡o?îß»‡*+M?î!ÆßM¿Ç?œ7®˜¿à}€(¯K³¿ìÁ=ÐE'¿ïÿßHÐSjUNASNone?ÈÚËyKØ?ůG1Sj?éýÉM!­
?ůG1Sj?Áõ1XED
?ÀyxØÀQ?낳©î®ý?ÀyxØÀQ?Ò××(ñ;?°ò¡Êg?æ"y"k‡c?°ò¡Êg?Ä
'Ó?¥ù|¿Tzg?êû}<ŸK=?¥ù|¿Tzg?û|ø?±¼Û™~¢?ï8#ïÀ?±¼Û™~¢?'Àú²oF?¦Zˆ"2$?ïiÿ16?¦Zˆ"2$?«/Ӊ'Ò?œê L6?îMÇRÿ?œê L6?•)æ<ç:W?‰·ú±rº?ïV°Î½?‰·ú±rºPSR4FGL J1712.9-4105?ê8Oä]¦é¿ò—7¿‰î+À:NM6êwØÀ;qäõ8@#Áåh$,?ý"B
y?Æȶè‰ì¨¿+L€ûµ?½YVˆwÞ3@cho«­?Ô´­Vœ¿ïùͶט?ïùÞHS'?³LyKµ¿ï€Ê`"?ê"ÄÀŽÐéUNASNone?ïàv®™A@?Ÿbò"…ÙH?o‰Qh—±?Ÿbò"…ÙH?ïÙ_c›c?Œ®bµt?s~PC3ŽQ?Œ®bµt?î‡tß-«?™ìh!@Ì?§ˆ²
%Næ?™ìh!@Ì?ïп" å?rô9ŸNk?w =ჱZ?rô9ŸNk?ï× ÕË?x¯ƒÌP?t/•'ûz?x¯ƒÌP?ï@½ÑËþà?¬E)r´"?—èEÈ7ñò?¬E)r´"?î*gÄN<é?Ÿ³K¦¯rB?­Yƒ¾‹Íp?Ÿ³K¦¯rB?ïqö%qå²?'K¾yµ¿
?'Á;JäÓ?'K¾yµ¿
AGN4FGL J1713.0-0521¿ìB@ƒeŒ@3	Ò9XÀ9±ZI!²À;Š$_ZÙj@_µ֟	@/«|,Ò?ˋ"ˆk?Ҝ"$'\@ob@ÛBà™Þ¿ßÞßHûG¿å¾»öº²¿ëò¢IkƒÝ¿åÈ7½±¿ïóˆ'	?íðh]a…UNASNone?ï®Ö¿ê¼!?­ÎÄnt?"JOü
Ì?­ÎÄnt?ïv…ÃMó?™
 §[Í?Œ¢^œêó.?™
 §[Í?î*iC¡¦•?·²€¾?­YkÁš½?·²€¾?ï¨Aê¨wO?qÈcz.Šy?…ï…`1?qÈcz.Šy?ïU6g4…?œåÄÎ"M¸?•Y3Oc?œåÄÎ"M¸?ëð²Òr ?Æ·Ù
Gׅ?ü=4¶7?Æ·Ù
Gׅ?ê›e"L9?°çÛµ·¡0?œêkvÏ?°çÛµ·¡0?ë5¿?°ñg°W:?ó+·¥–?°ñg°W:AGN4FGL J1713.0-4236c?êxßÚh
RÀˆãƒÈvýÀ9t«ášº+À:Î	ԕ+@ Q(;³_@såÍNÓ?ÏÔ߀Xªç?Ïo¹vXÌË@ía¥6…Î?ýZ
…#ÀÏ?ï:`Nq¿ávŸLa¿ÜI@¢B¶¿ãy[k`¡+¿éÊìW¬@¿ïóGŠÙvUNASNone?ì­D>'$?Á}Ûßœ?º•ÜîÝ?Á}Ûßœ?êÃÇëf•á?ÃtJj1w?ÄðàRe¨{?ÃtJj1w?ë.ÌîIŽ?­4ÒN%F?ÃDÌFÙÇ÷?­4ÒN%F?ê‡Ëg‹Ä3?¨¬Xð²Š?ÅàÒaÐï5?¨¬Xð²Š?à:`ûmt?Ëoƒ__Oá?ߋÝ>	%?Ëoƒ__Oá?ܨ#(èÆA?ӈ…DÍåQ?á«îk‹œß?ӈ…DÍåQ?á ¦È·Ú?¸×˜*·AS?ݾ²nbðK?¸×˜*·AS?Ì|=õü=u?µbGx?èàð'€ð£?µbGx MIXED4FGL J1714.6+3228?à[ídz†Œ@@ÆÂT£ÆÀ;ª{jÚinÀ<äŽ^Òô.@!õè?û³5L'?Ñõ£KÛ¡?²º·¡lvÌ?ã'3¡m"˜@O?w9Gt¿ï îzÔ]?ïò®Þ¥<e¿Õ'*g2¿ïá.žxük?ï–kFŸ÷'¿Ü¾ïÿ×¼UNASNone?ïÿœ^V2Î?
^(‡:?èp»9?
^(‡:?ïñqda~?l'õö(F?]៱"…?l'õö(F?ï"Bö"g?zª¨üM?ŽïyÌ©ú*?zª¨üM?ïÿ›Žâo?:¡²qÏì?	'ǽ?:¡²qÏì?ïþ'Ü‹(4?1Š€îÆ?'Ò3%(÷?1Š€îÆ?ïɒ´ç‹?ÂµE»W?{6¥r±ž?ÂµE»W?ïWt9I?'Lږgt©?•xÖÞý?'Lږgt©?ïýQSH–6?=ÓòGšÐ?5ugvh½8?=ÓòGšÐAGN4FGL J1714.8-1421¿ã_û>éäz@+·+ˆDÀÀ:™âàíÀ<Fƒ
â@Rzé*?úË$£Mx?׈†KÞû£?áÂZ£Š´@E܃#6@AmÙ!næ¿ï""Ÿ´»´?ïýuÁÎ#¿ÚñÞ"Š™¿ÕÝÏßäØ¿ås‡ìÈ뗿ïý
a½_GUNASNone?ï±^5%·Ü?…ßÖâàÔ?ƒ¨r²r?…ßÖâàÔ?ì28¦(?Ä`ØÏ`P?¿în:λ˜?Ä`ØÏ`P?íŒÉæØ*"?¡'Û£:"`?³™°Ç†Ýl?¡'Û£:"`?í¯¾r}1??'Ñ%†~2+?²'n<7ƒ?'Ñ%†~2+?î)ÛØÙ?°/Fk¹ù?­f.-öïq?°/Fk¹ù?஽)Ÿç?ӚeÊå?Þ¢…­öÀ3?ӚeÊå?ëŽ=*Ì?®Ô‰}z|?ÁÇßWÏ?®Ô‰}z|?çÖÐ[Î?·è·øå7?ÑéÆR_He?·è·øå7AGN4FGL J1714.8-3849¿ì"üÛ¢…¿ÀéÕÖX½À8@NÕP)
À9Ì:䜸@—áŸ@2êRï'?Áùh6J>è?͉—Bý*¹@Û%ö3Îd?úX»¾¶S?ï¯Ö燿åÌÞý';¿àKeè'%¿åìŒñª²¿ìV/n¿ìêßBEJUNASNone?Ѝ®ì^"è?ÐÂ{ü‹èg?ç¹(‰Ð½Œ?ÐÂ{ü‹èg?ÏiÊã­RÎ?Æ{S%ñ?è%G«M?Æ{S%ñ?ÕÊbÑÓ¿'?´tS],¬?åΗ m?´tS],¬?Ì
m—æ?±k£ñ›À?èü¤¿:G?±k£ñ›À?·Oú…•÷;?˞Ǵg®Ã?í¯GY?˞Ǵg®Ã?›i7÷ÊÁ?¦÷!6¿z?ï$¶@sê?¦÷!6¿z?¸™8SÏ"!?¦ø(‰û°ª?ììØõ"Ú,?¦ø(‰û°ª?uãžÑZ?lчm"TC?ïÔ9ⓢN?lчm"TCPSR4FGL J1714.9-3324?ævq€ÇÞ@ö¥
k#À9oNäHÀ;*¯ÿ6¬d@ÅÛêÌçû@òzÞÃo?Țk%½Ô·?Û}¶Äͤä@5" ¼8?óH}ˆkI?ÚZÀÀÏéb¿ßð½Âôu¿ÜZе
¿ä3ò«ƒ¦é¿ìl¸?wT¿ïþ'¼ÞB@UNASNone3FGL J1714.6-3327?ÅþŭɧS?›FÜ¢?ê€N"–+?›FÜ¢?Ãi'xŒP'?¾vA\¹
ð?ë%¶!Üëö?¾vA\¹
ð?ÖØÙ?Ìɝ?²ë`kz¢^?䓓`›2?²ë`kz¢^?Ðû´.£ß÷?¬ò
閔Ô?ç'%è®?¬ò
閔Ô?¨Égëá4ð?±ö$X%»8?îsixæq?±ö$X%»8?‹îÚhÁµm?"ÿC­Ùák?ïD–\ù*?"ÿC­Ùák?²-J¨''W?¡*€>ºâ?íºV«2sE?¡*€>ºâ?ˆY?!Ù¯?tb!9ãßå?¯•?tb!9ãßåPSR4FGL J1715.7-4239?î_ð;ÍóÀðCRe(À9ì) ã9÷À;­e(xÅ@¸dC¡j@õÆÛò¾?ЂV¼¥7]?°	ž¡l2?èk¤Éx"v@ٍ\õNv¿Ûàÿß"?ï¸x·¡Â]¿è3¤Ýšzj¿ëU—Ià?yë‰%ƒU¿ïÍõ´L£UNASNone?ïé­àš×T?xŒ3œfó?fRtFô:?xŒ3œfó?ï×[*6ú?';`Zá•?tRjì#w?';`Zá•?îÅ~d^ú6?™Ƈéaç?£¨¾[ߔ?™Ƈéaç?ïöΌ{µ?Cșö	[¤?Rbç'8?Cșö	[¤?ïIQÌÀ&e?¥¯=?–ÕÆaûh?¥¯=?îËt2µg‰?´T@lSPº?£H¼×=<l?´T@lSPº?í "Ý{=?§ú`¤r ?¶û_Ÿ\X?§ú`¤r ?@¬v?‰"³çÓ­I?Z/ÔâxŽ?‰"³çÓ­IAGN4FGL J1716.1+2309?ÞÊ8/=Җ@>§T~–À:}ÜygËÀ<~¾b¦¾@ 4‹Âktî?ü‹vUDz²?Ä1}{€Õ?ÂFÒâ»vŽ@F}ÄY?ú<–÷RÝH¿ïiaB?ïÿîbHÊt¿àVà¡ë͙¿Ég]äâî¿é
Ä^ê<¿Çâðµ	UNASNone?ïìê
î?fe×"†~?cô®˜zO?fe×"†~?î®è€‡yÜ?°˜'ïƒ?¥wù@07?°˜'ïƒ?6;?ˆÕhbü	â?¾ƒ«='?ˆÕhbü	â?î0òVR?¼gW=ù?¬ÿÏѶâ?¼gW=ù?î:
U‹<?ª;g§\?¬_Z«ã—@?ª;g§\?éb}BmZC?ÍCE§ 6?Êv
öJ–ô?ÍCE§ 6?îné°ï\Ö?ŸP?Oϊ½?©dôyΞ?ŸP?Oϊ½?ç®Ö–"ïz?¹à"ªÌ…?ТRÒØ!?¹à"ªÌ…AGN4FGL J1716.1-4342c?Ù<£›oÜÀ	U°5½Q/À9§>ïÿ×¼À:îfWLíï@~Êö†@¿–áXu?ÒéWG²J?ٗ֠áž@
/Â=&Ñü@-ø¦š^?ï
užèó¿æ"_@Ø7¿ä˜=Î펿ëÉZQ…-Ò¿äس|
¿ïÿäÅøUNASNone?íPù¤[È?º:'o{/?µx7œ"ï½?º:'o{/?ê=/ñèì?Áæã³\ý÷?Ç@8\ñP?Áæã³\ý÷?êÿ]Rbð²?«m³þóÜ?ÄŠ¶t=6?«m³þóÜ?í=ˆH"?›–½˜½«¼?¶¼߀?›–½˜½«¼?è3¨üŽ'?Æ	Ìã¿?Ï1\
Çé¹?Æ	Ìã¿?ÌGFëˆ?̳c½à?èà..E?̳c½à?â¤Ouç–Z?¸2px_£"?Ú·a0ÓK?¸2px_£"?Ӌ"×à?¿÷բΙ?æ:n"õt?¿÷բΙ)MIXED4FGL J1716.9-4152?íAIò<sÀÖÆÞvB|À9½laR*oÀ;"÷í@'qÓW@7"¹hkú?ÍWÙu&É?ʧ"Är¶+@j <¶i´?û†2(œ+?ï5¹pޏ?ïg,_›–¿ØÝZ»g¿äE‹àsr¾¿èªÜb§¿ïþîB=g?UNASNone?î¡R¶`?«¤IcDu?¥êÔ£šè?«¤IcDu?ëø: H†?½Ñ°ª_î?À»~Ýè?½Ñ°ª_î?íö7Grð?Ÿª4´wj?°NEÃ!¶?Ÿª4´wj?ëªRê¼)š?£Qœüë®?ÁV´UY˜?£Qœüë®?å»t}UkA?Èîgm2Ċ?ԉU)}?Èîgm2Ċ?á8îÌ&Ó?рßè¢/.?ݎ"g³îZ?рßè¢/.?äpc%¥g>?¸™qŒˆ?×9´µ1ƒ?¸™qŒˆ?Ú47n¨C?ºA='IØ«?âåä{È«Þ?ºA='IØ«MIXED4FGL J1717.0-3218¿×Z‰»w‡B@
WýO0ÀÀ9älòq¢À;6q'Šˆ…@ íãLì@¡ÞËÒÒ?Ã*[sCD¿C10ǾZ?¡ñ,}ŒrÀ@Õ®zÒ.6¿ã'㍲b?ïœ)@ìt¿å,"½ð¿èó`_fAþ¿èkÆ¢'9ú?¸ˆ_	¥Æ#UNASNone?ïúq%º­C?JHp‹Œ‹¼?F;iÆPl?JHp‹Œ‹¼?ï֘	?…lÀš$Þü?t³û`Ü(R?…lÀš$Þü?%3/?‰ª³#V¼è?6¥uÉD?‰ª³#V¼è?ïòגðÕ?Jt*Ťö?[üQÔà?Jt*Ťö?ï—ÃWÐmã?êŠ:?Š)þ&3?êŠ:?ît»›Ìúš?¶¥-"ºq%?¨´FD=^?¶¥-"ºq%?î\½µ?¢Ð+3Ü?®ÏŽÖĈ¶?¢Ð+3Ü?ïž&5–1R?¯çì:^Ì?ˆvr‰EŸ®?¯çì:^ÌAGN4FGL J1717.5-5804?ígšlíÀ'hRÀ:kàèãƒÈÀ<~Êx_@G2?˜F]?üX#ã4_?ÊÚ*BôœJ?èð¾C
Â@5I¢
c@¥®¥ÅL?ìMIÊNmK¿â¡Ý_ìû¿•ˆÞWÜ¿à8IÝï‰æ¿ïÆd""T‹¿ïý	«zl®UNASNone3FGL J1717.6-5802?º5çÐUº¿?ą‰ñ9?ì¹CõH¨?ą‰ñ9?ØãnJœ—Œ?ȦĴiB~?ãŽHÚ±´:?ȦĴiB~?ÒæW2üÂ?²38ÃiA?æŒÔfõŸ?²38ÃiA?ÛUޅÿ*d?²
±bpßý?âU½jÎ?²
±bpßý?ŸpÊîPU-?¦eU"\?ïy¨Ò5†?¦eU"\?²zO"¦=Ú?·}ÍÜerÖ?í°¶¸öµ?·}ÍÜerÖ?¿^ÅÈ¡™î?©'Þ{¬æ×?ì'FëÌÂ?©'Þ{¬æ×?´uš‹Üí?¡Rîb¿?íqL®"bP?¡Rîb¿PSR4FGL J1717.5-4022¿ÁnÈ=Nž¿÷SŒdý±À:–Í[h£À<Br©jÈ@ B–áÙNe?ÿƒ\=¹?Õ2køvžÃ?ïùƒ^ıu@á¹Þ³?ý:˜‡ É¿ärâ?û˜'¿ïÿä†ýµ£?ïþú·Šñ¿Ø‹*k
•¿ì°¡óÛ/¿ïé˜_‡ÏîUNASNone?â&(j¤°ñ?Î(q@?Û³¯*¶ž?Î(q@?àéûR,ƒÓ?ÏpÐÖœ?Þ,	[¦øZ?ÏpÐÖœ?å@‹ÓTȧ?²_í&tä?Õ~èYVn³?²_í&tä?Ù$Þ¼cs?»Í†¯?ãm¡ÎFu?»Í†¯?×c‡š¤Â©?ÏíX\ëò?äN<2­ž¬?ÏíX\ëò?Àe¿el°?ƋÈdwÉ?ëæ;æ¤Ô?ƋÈdwÉ?׶r
ʪ?·™"'Ù÷?ä$Æùªô?·™"'Ù÷?¶»/%üƒ?°™ZԀÙ?í(šֈ@?°™ZԀÙMIXED4FGL J1717.6-4404?ÏÙk@ÀºpÀ¿¸fä;À9"šv8kÀ:Ûµ#bۗ@f_>ÿÅ@8Z\lèa?ÒI䥆?ÕޏÂÖ(ì@Dy¬"H@n"³*å?ïüPþ .‰¿íQ9®ww0¿ÞJªž#Áü¿è¬Fàˆ¿ë•¢ß='³¿ïúÂÇ;=UNASNone3FGL J1717.6-4404?îEe'€ö‹?³´Õ;'$?«©¦ØÌ~V?³´Õ;'$?îÉñÉÌ?§:ƕ:
?£`îÌ3ÇC?§:ƕ:
?é"çJHð×?®Êq$pÒÅ?ɬbÖÜ<¤?®Êq$pÒÅ?îbiþ» A?¡'‡7´{?©Ù`Mûó?¡'‡7´{?åýˆ<,´?ȯÏpÁH?Ô–Ç?ȯÏpÁH?é5-þ•ó?Ël‡‹0©?Ë+—H¨6?Ël‡‹0©?å!Aù÷?´3ð8àçÏ?Õ¼Å}Î?´3ð8àçÏ?âgµ°ÝŒ?¼b´]È»¤?Û0•þžDé?¼b´]È»¤AGN4FGL J1717.8+1955¿å3]oÐP@=1	¾ºÀ:Ë:CȬ­À<bw‰¤Y@Ú Gs1@éºÿDï?¼Ö_Æ?"žgšÕ*?À†D}2…¹@¯Sj5S?CtÉÖ¿°Å'<3¿êþ'âÆ3V¿èdµVŽ'¿«d]D 7пè™ÇâWMšUNASNone?ï÷0®£?PcQå0÷?Qžà	Fã?PcQå0÷?ïèÑ삅è?uB\½]S?g.¾¿´?uB\½]S?ï³äMia»?|"kªêð?ƒì¤G¹M?|"kªêð?ï÷$ARۚ?=ÞQ£'°[?Q·|Û×,{?=ÞQ£'°[?ït8~¡›œ?'ŒWcT"?'xð+̌‹?'ŒWcT"?f?–£(8®GQ?‰ú¿€1^_?–£(8®GQ?ï
Ûï» f?–iºõ-ë?ž¤'d‰N?–iºõ-ë?ï¿Êx^¶o?tQ 8žœÙ?€
aØ,:g?tQ 8žœÙAGN4FGL J1717.8+3925?ßfïç¶@A†
¢À;Uî:ތÀ<ɓnÝ-m@ ïñ2@º­,**?ӟ¡[¢?Û>.cëŒÖ@û$ p¸Ð@¶ÁȌ̿ïýíÁ?￧¬_o¿Äó¡ã?*¿åB˜Ì@)¿çï…^y2¿ï¾­àMˆUNASNone?ïñ \4?W_±B?\¿GŠ?W_±B?ï'Ápºß?" ð§§·/?‹O£ïBtm?" ð§§·/?ïU³øâ̶?‰WFOÿù?•I€çB?‰WFOÿù?îàqÍçn?‹;'wþ?¡ÿ˜ái»%?‹;'wþ?ïĞwú¸m?~Â6Ššg?}°Ä 0m?~Â6Ššg?îL@â?È?·˜}uš¸ˆ?«>ûîlg"?·˜}uš¸ˆ?î3	%ÑÌ?ŸÐ˜çˉ^?¬ÏnÁ@?ŸÐ˜çˉ^?ꅩœ¾^—?¬8¸ž?ÅéY…£?¬8¸žAGN4FGL J1718.6-5821?êöÿ¨rÀ'ø@À:
ùûAÀ;ǁ]b±¦@Õ0‹yp@}G8£µ|?ÁÙ¿¤p7K?´hÊCÛw
?ðŸ-݈ܳ@•»ô7tá?ïÆTdÜ#¿ãªÛuÜûï¿æî!7¿äNMÃiÍ¿îÐüqÖ1¿ïîDنUNASNone?ïá£,¯$_?f›ÍÉ"m?n\Óm¸X¹?f›ÍÉ"m?ï¿'bš?‹Í¯1´‰?€8633?‹Í¯1´‰?ïFÒ]–šG?s •š?—%´Kté#?s •š?Èw
å?o£-&Úz?‰Ué¾Ì?o£-&Úz?ïn7ѱÀ?t5ˆ­K?'9Âþ?t5ˆ­K?ï1Ý)2Ì?§GºõLg?™Ýd`"?§GºõLg?íœQ"à5ú?¤›™2_?³s`þP0?¤›™2_?í#4î§ÆŒ?žó:ß¿?¶æXŠÁË£?žó:ß¿AGN4FGL J1719.0-4038¿²níJ
¿ýeÙ($â8À:|Í°ø[À;JuòËd@ µY€.@aøDIÜ?ÇÚDºõŠ?¦C®Öl³²?å>ÖÕdK?üAòMå¼?ï­o¤Ó‰¿çN>f˜¿å<â¿'r¶¿å]'«ŽŽ¤¿á£Ž_©³Ã¿ß1ßá|‡:UNASNone?ïømÜɼn?O±D4¹´í?NHŒ©:´?O±D4¹´í?ï¨='±9?›#§ªh?…ðŸIbÈÃ?›#§ªh?ï°Æ^+ƒ?€UËÖYÕ?ƒÎhkîÍh?€UËÖYÕ?ïÀE&>œã?eÉøû⋑?ÝlÔRöÈ?eÉøû⋑?ïì‡Ç×fü?`©ÁÈ?cx8<ì+?`©ÁÈ?î?Qva¨‰?·¼ðbˆsG?¬
è˜-©t?·¼ðbˆsG?ïY±w0ä?•[›#t‰?"Éԉ|?•[›#t‰?íóґ'?¡Vr+Û>ï?±âakw>È?¡Vr+Û>ïAGN4FGL J1719.0-4221?ï
äAôyÀ v}4ßÀ9Á•XÂ8õÀ;A	pÂ
@>nfë@C{Ó?Î!4x®?܉+bYfy@LeáÜ(Š?ök¥¥–}?ïmq½²}–¿x:ì1ŽdÕ¿åYxâií¿è— Ÿ²¸¿ëɉDH"¿ïó<7¾³/UNASNone?â "˜8ùú?ÎB<\ôïù?Û¿ºÏŽ?ÎB<\ôïù?Öc‹ïý?Íi¼‡/^½?äñκ?Íi¼‡/^½?ç:pÌ_ ?°O@¥¤¤?ыgÛAÁ?°O@¥¤¤?Õ7"9ì?°•hY?åd=ò~ã
?°•hY?ÒBÝÅÃn)?Ëæj~<á?æޑHë?Ëæj~<á?­ì'7k_?¹¤[Èp`?î!6Ü`º?¹¤[Èp`?ÉBý9ÀÚÀ?°µ˜Ä˜±ù?é¯@±ÉP?°µ˜Ä˜±ù?‹£ø;g??xl€½oÙ¢?ï"ÅpHM³?xl€½oÙ¢MIXED4FGL J1719.1-5348¿ïvi?x²À"¤w¯dÀ:hRGËp¬À<¿¨!Ù@…"|NZ+@–žh5s?¬Gq-À?@‡1Ó?Ñ´âË;Ó@×nŽ¨ú¶¿îJj½
<)?ïò§½HËK¿Ý·DdÞÑÝ¿æ'Ê !Èþ¿Û#¾…â-¿à9"¿ºëyUNASNone?ïø:ñò?FN[cÆ&?O9sÍ´?FN[cÆ&?ïçÇžmG?vZ*Ö[Ù}?h~8 Ë‰ ?vZ*Ö[Ù}?ïÌ/ÑSð?.ƒd°·?yè:‹'?.ƒd°·?ïóÂõ³uä?CjÜQœe¤?Xz%¡Y<?CjÜQœe¤?ïÚj̞öó?k°˜OËÒ?rʙ¢Æ?k°˜OËÒ?ït]¦èüG?¥Q!P—#?'tK¹
"?¥Q!P—#?ïuž<Á|?Ž›I%ç/?¢˜~ŽÕ?Ž›I%ç/?ï¹PŒÆˆ¡?t˶ñôò?«ÜÝ$)ž?t˶ñôòAGN4FGL J1719.3-3424?ëü¼‡7õÃ?û!Â]BÀ:d%B{¦À<¦Á Hà@ƒžçŒ@Á@ľ
'*?ՈŽÄÔZá?ïú›ýwª@'
=p£×@Âè/SՕ¿ä‡Úà
í¿Ó§üÞ¸\¨?äz؍Út¿äém
A"¿ïüª£´P?ï@ôQvYUNASNone?àâÙwÑä?НŸ@U?Þ:Mð\8?НŸ@U?æÝIéûS??˜€-%ÁÊ?ÒEl,	Y?˜€-%ÁÊ?å±t`hå6?²NHÔ®cB?ԝ?.5•?²NHÔ®cB?äHn™:Ï	?¾ˆf–b?×o"͊aî?¾ˆf–b?ǬRM•ú?Æ,2FxF?êë~,š'?Æ,2FxF?ÂÄd솯?ƲŸø¶é?ëNæþ"ÞT?ƲŸø¶é?ǂM,ƒ–£?²jÜõ8?êl´ßW?²jÜõ8?Àškuø]?µW£…E?ëÙ\%"é?µW£…EMIXED4FGL J1719.4-2916?›nÿ†Tç@n"$咖À:Q'l~®\À;UÎ{"¶
@!uÇ,yÜ@E¦'¶(F?Öââ7î?Þ¡x ¥§o@ ˆC0y@YKË°m?ïR…sq礿Ý]+4¾y¿ç˜Æ‰ˆ*¿æ¡^X¿îÚÑb2Ð¿ïþ*ÝúºUNASNone?ïL`R
Ã? Ê~­žÎ?–sõ¿6¤? Ê~­žÎ?êe­BÔø?ÀlW…ç¤Ù?ÆiÁJô¬ ?ÀlW…ç¤Ù?ìþY;c6?¢)ö›î¬?¸M7nÀÎ?¢)ö›î¬?ív;ü/ç?˜V){{*×?´N §'Ç?˜V){{*×?훙óþâ@?´kIãÄx$?³#0`äÔþ?´kIãÄx$?ÐɃÔWÒò?̦vvÔȚ?ç›>Ô‡?̦vvÔȚ?ãqóåaæq?¸Jt²ùIÕ?Ù5<3?¸Jt²ùIÕ?×%"BÜb[?»é£OÙe?äm5ޑÎÓ?»é£OÙeMIXED4FGL J1720.1-4358?â
ܞ?àZÀ<Á^ڀêÀ9†¿:¬¤À;$G4q÷"@á›þMÎ?@…ÜMsP?Æ[yMsÑ?ºþv½÷qç?øýÎè/ÿ¢@9öw– ?ë0¿e†?ïx5›Ã?…¿éJº¾­OY¿äËZ;µ¸´¿àqÁŸ:¿ï¾ÿ—$tUNASNone?
U9T?­É‡ÛNJš?‰Ô|µ?­É‡ÛNJš?ïUэ? V¬Ã>?•\%Õ-—³? V¬Ã>?ï3¡†^9­?'è[T¬®?™‹Ï7¨fP?'è[T¬®?ïIQ	ÝÏT?€JúÁ§?–ÕÞ¿«•?€JúÁ§?îe/Gså‰?ª£—=VŸ4?©­ˆÁ§w?ª£—=VŸ4?ìu•qƒ×?ÂHνº?¼STwáF?ÂHνº?ì"N}ÞÊs?­6
Ìÿõ?»ÝŒ	¬k?­6
Ìÿõ?ê/LQoçÍ?³¡!쯃J?ÇBκ@`Ì?³¡!쯃JAGN4FGL J1720.6+0708¿é‰§wíf@7kDå^³À9×Ùµ›äÀ<àŽJ°þ@´fêD×Ë@Yܚ )×?Á#Q(f¦}?Ù é¤@ŸË':)Ç?þ¶§NŽ?ïý$ƒmj¿Ñô;[uǂ¿áäÊE¿ç|卍ó¿ìÞÛÃ	Õl¿ïä1‹@UNASNone3FGL J1720.7+0711?º¨¾ÐŠÇ?¾äÇ|?콊è%î§?¾äÇ|?ŏװÍà?Àɓg%~?êœ
̇û?Àɓg%~?Òaò°®€?±é		Z?æñϧ¨À?±é		Z?Òµ¥Ïîü?­²°o]«¹?æö¥-'?­²°o]«¹?‹õ´ûßYÎ? •ƒ°/O|?ï)+وÙ? •ƒ°/O|?
6;…¥?¢ÙϵLŒý?ï®MìÙ?¢ÙϵLŒý? /£dcv?"Ò1¯ˆ?ë?îýÏ¢À	?"Ò1¯ˆ?ë?™!C<WÚ?†o$'_?ï7fö?†o$'_PSR4FGL J1721.3-5257¿Ýb¾"Xo¶À"AiÂ;ySÀ:%ÛÞ¸‡›À<$"û¥'l@
5]/@ô·Í?Åï"77y¿?ãªØ¡e@ëÒú
w¸@Ù¡û½Ñ¿Ï2þ'W¿Ý×&¢¬ì¿ÜëÀ š¿é_îbHÊt¿ïôù è­Ô¿ï%m
ÊUNASNone3FGL J1721.4-5253?Ûk`ę€"?ÌÇåÎ6À?âJO³?ï?ÌÇåÎ6À?ÛF‹\6"?ɐ¤èØ5?â\ºQä½ô?ɐ¤èØ5?ÚâË"t'?³çäXVC´?⎚yµÅí?³çäXVC´?ãÉhk?­[	42ìÏ?Øm/ÅâÅ)?­[	42ìÏ?ªš‹ÍwC?Ááhvr3_?î_–W^¥l?Ááhvr3_?°Ö×ÖíÂN?·å«¿+¼?íå%‰F?·å«¿+¼?­XlŁþ?œÞ-7ê©·?î*y+?œÞ-7ê©·?´îÔuTï/?ž9îm™Q?íb%q~j?ž9îm™QMIXED4FGL J1721.4+2529¿âó]òÆÓÜ@>?§e47?À:sÿÜĒÀ<DTž½ÅÉ@Œ¶¦Å§@æù[¡†?¤#
q¿¯—%ÿv Ï?å&-'2ÂË@ú 
÷Õº¿ÓÀŽ%D.¿ê–-žž¼¿éÿ7T*$¿çñ"'›¿ãæþÜêQB¿ïæH¿™UNASNone?ï÷iI€ã¦?gKXÏí-?Q-m,óbí?gKXÏí-?ïé‰:É!?ub‹Ïý9ï?fvÅK|"Ì?ub‹Ïý9ï?ï"Y'ŸWÒ?‹ÔYü#;>?Šé›'JÓ~?‹ÔYü#;>?ïódLõjê?DDHþžé?Y7f\¢
¶?DDHþžé?ïãk=®?tœ.;S‹?lë"Êè*?tœ.;S‹?ï¤	qe?l?Žé?/{ÿ¼?†ý£´n"Û?Žé?/{ÿ¼?ï}%ñôÏ?,;žñÛ?[AäÐ?,;žñÛ?ïqKµò&	?ƒE6
Ûn?'Ö‰HšvÚ?ƒE6
ÛnAGN4FGL J1721.4+1131¿×ÉUSÄx@@9$ƒÛÂ3À:Eóå?ŠZÀ;íåf ÆI@dˆSöø@('»0Ã?Ä\|,Ì<?µÛ.dlf?ñúÑ!Æ#e@Ley+ü¿ïä:Âs­w?ï´êB~¸¿â7¨ã¹x\¿é¡nD9Q¿Ü4Â_5š—¿ãƒö.Åæ)UNASNone?ïóŠö,†`?S) x,ß?Xêöª0^?S) x,ß?ï¹$æX'ù?Š|uÉ;?¶ÆZ×¹Ó?Š|uÉ;?ï©Yk3Þ2?€ê%<kfd?…©¥@ÆãŒ?€ê%<kfd?ï½`«'hÉ?f Úy?€§ÕVùé?f Úy?ïÝȸ?‡ÛSþMÛþ?‹È»T±0…?‡ÛSþMÛþ?î7[÷o?·{ÆÛw?¬Ê=õZÀ?·{ÆÛw?î™0Œ©Ší?Ÿ
y‡Ú?¦l÷1÷µ3?Ÿ
y‡Ú?íå'šë?Ÿ½bŸÓ?°ÓoÙ)?Ÿ½bŸÓAGN4FGL J1721.7-3917¿ïÛ}ä ?T¿÷ÝÚ;JXêÀ9Pè0-À:ÝîgQGñ@•8"Djé@7褙§Ü?ãRÿ" ?Ð÷Šûñþ`@À ìߒ?ûË …¸Ò?çi·ßTä´¿Úzµ]šdñ¿å^ê–p¿àuT«Rÿ¿ð?ïþ¥¢fqÏUNASNone3FGL J1721.8-3919?äñ°—  ?ÏLã+D8?ÖžÑç¾Á?ÏLã+D8?ä÷89ò?͗ô}ë¾*?֏Œùþ?͗ô}ë¾*?æ³¥Ó±?³b²Q^\ü?ҙô´Xâ?³b²Q^\ü?ê8‰SÔï?®]Єf?ÇÚ³Œ¬C?®]Єf?Émì™GÃ?ÇðV¡™ºž?餄úÙ®?ÇðV¡™ºž?·2%#Šz–?Á¡—õžq?í»[œo?Á¡—õžq?Ìt ÌúÖ1?´=zl<E)?èâ×ÌÁJt?´=zl<E)?Á:]Ù,µ?°6]f'?ë±{h‰´Ó?°6]f'MIXED4FGL J1722.1-4007¿çÌMyÿ©À*¼¤¡5À9q¼´i)À:þX"»@=ó~'W0@µiF·G?Êl‡"?Ŝ¢x†0@Bõ:ªú@ͳ\cX??âøC]¢Èl¿ÜQ0^ƒ¿ä¸Çâ'@¸¿âs,þåÑ¿ïOÙ\'H?ÔVˀœUNASNone?ï›êWÞIˆ?"Š\öâ0H?‰j,
æ?"Š\öâ0H?ï`þ›ã0?¾®÷?"à,‡Õð?¾®÷?íŽÒ9âé‰?¡f;"v­í?³‰n2 ¹?¡f;"v­í?ïS€±øA?|gáT
?•éß°"×?|gáT
?쪽®?¼–UŸø6?¿ç_ŠªŽ?¼–UŸø6?ëÐ*áfH?Æú4,Ð\?ü¿Tzfà?Æú4,Ð\?囌šÏñè?·ÑaSN?ÔÈæÊ`1?·ÑaSN?è"{kA}µ?³­Pté_J?Í®Rú	,?³­Pté_J
AGN4FGL J1722.1-3205¿í'+årFU@Mt­P0À8Ù¤K¤CAÀ:³*dW˜m@ñ+:ÁG@ø¼²£V?Õ²½?É[¼>_@a~4¹E1?û/-4k—~¿ïr> wæ?ïýéÚúŒù¿èÄ¢'ßܿ䅠ž²´¿è)ó¹  ¿ïÿ´ìw8UNASNone?íà57¢â ?ÀϛÊÚ@?°þVBzû~?ÀϛÊÚ@?æê®áÜ?ǜY_?Ò*£Ì<Gô?ǜY_?è_Bó<®?²a'kÀü?΂ô3™H?²a'kÀü?ê©JÀSÓÎ?¨Ã͖=?ÅZÔþ°°É?¨Ã͖=?ç-~õ˜6Ý?ƖNô¸VÒ?Ñ¥ϒF?ƖNô¸VÒ?Êb¡ ã?ÊÅê5b/?égW¹¿Ç?ÊÅê5b/?âŽ	˜…?´ Ÿbj?ÛÖãìÎõÇ?´ Ÿbj?ËöGî3ØR?¹Š—ä§?éns	ë?¹Š—ä§MIXED4FGL J1722.6-3135¿ïå¦åd@¹^ƒCÿÀ:m^º z^À;üVÈc±€@XýËrYº@Ú³R¨D?փže[N…?îù¶9ãP@Z5Ö{¢?ÿ‹Þuk¼ç?ًÛk¡¿è×n~ÓE¿Æ~h»«<Y¿Ü	ÆTㇿïÿý{ÁA~?h$¬ˆUNASNone?ß={q̇>?ÑR-EÊ
?àaBG¼a?ÑR-EÊ
?ã@ÌLãø&?Íø …qœ?Ù~gf8³?Íø …qœ?å多²&?²¹yÑÛ²÷?Ô4¶Ê›³ê?²¹yÑÛ²÷?äP2"Ê?¸ò
T.åÍ?×Í_šÖkÃ?¸ò
T.åÍ?Ùlي—7?Ô/(Šk[÷?ãI˜«:´d?Ô/(Šk[÷?¯¼)ƒµk?¶ÜØ°@l?î=Z9?¶ÜØ°@l?С	ä²?¸m\ʒR?ç¯{z
§?¸m\ʒR?µè††]"?©®oqUli?íBï/g?©®oqUliMIXED4FGL J1722.8-0418?í¹b"·Ç@1z¿¹¾ÓÀ9£ÎµÛÀÀ;ƒ¤Ùš;@Žy&²qW@òÜ`¾†¹?¿È`g¯ù?ȑXJz@é{f¨«…@d]!Ä ¿ïúþ8£N?ïþ|¿á
Æ,Ÿ›¿ç?!þØb­¿ä…ºŸM¸›¿ïÿõMõVYUNASNone3FGL J1722.7-0415?ë}`Cj@™?À9IºUž:?Â
~òVý›?À9IºUž:?â…×Ѓµ?ÏÙÕ/-%?ÚôP_úø•?ÏÙÕ/-%?íÝEô^•?¡rçíÔH0?³ÒÙX?¡rçíÔH0?éK§ÑÉ>€?§÷.!à×D?ÊÑ`¸Ûþ?§÷.!à×D?àŒ¿
?ȧH#ôì?ßøæåÙõ?ȧH#ôì?Å[÷¬¼?Ëvftå@r?ê©;TÐù?Ëvftå@r?ägZ¾M¿?¶Ž}1F-"?×Ç1Jƒd'?¶Ž}1F-"?É=¦©¢{?´$LPëžØ?é½ð–U—a?´$LPëžØMIXED4FGL J1723.1-2859?å4•3Œ@_\ÔmÀ9áºu²3ÄÀ;U';&F¼@¤š"i©½@ùB%?Ò*5}æ4Ó?ß<eáÜ)@ÅSü×V"@ña£Êu?Öû{8…ƒ?ïäÕ!…
ì¿ç²™0¬¿è:P(6ï¿ë»¹.׿ï®
4»ÉUNASNone?íE:'îîq?¹J
©ëæ?µÖ+笥z?¹J
©ëæ?â¢{¹ùzD?Êþz"€Ç?Ú»Œ
y?Êþz"€Ç?êOôÑððe?«Æ(Â秷?ÆÀ,¸<>l?«Æ(Â秷?éÃxÁ‡æ?¨eX*€µ‡?ÈòûÁàh?¨eX*€µ‡?ærñ¶È?˽ÿ™AŸ?Óöܒp?˽ÿ™AŸ?µg‰´Æ²?ºâ‹îéµÄ?í]3 +Ú?ºâ‹îéµÄ?Óv¶È 1?·ô"É͞A?æD¤›ïùç?·ô"É͞A?ÅQ†å,ž?°³`…?꫞z´Ù?°³`…MIXED4FGL J1723.5-0501e?ⱟk¯jU@0ös>»ýrÀ8¥½áw~½À;Gýœ@ sÍ$™g?ÿæI ]?­'—¾V迅'LmcR,?ÝÉn"æW@BØ(J¡å?Փë$%Ï¿ãÎý'¬¿ã©yámm¿Û1¢åGÂâ¿âCuÀÌcp¿ÆÑM$ ô,UNASNone3FGL J1725.0-0513?ïÜILO8ø?pMå /:?qÛYõð'µ?pMå /:?ﯞkîï?'MkØ;!?"eb'á?'MkØ;!?íëýa•[?£ ÑS;³­?° ô3*?£ ÑS;³­?ïHÉÖß[?'PÆqáë'?–æÅ%Ì]à?'PÆqáë'?îàq0^? ˜°¡?¡ÿÎè&? ˜°¡?îVéÌ ?³»ÕÿL?ª'c??…ý?³»ÕÿL?î
9þ3S?¤ì‰|QE~?¯\` x±È?¤ì‰|QE~?í,ËÂ-.?¢í¬h?¶Ÿ‰ 6Ȓ?¢í¬hAGN4FGL J1723.6-4126?¸†•[Àž'6§À9È.5p¿À;/51:4¯@'')Â@8M[Óem?Îàw	KÙ?¿ƒ"´µÕ?÷ÞêÁªYÛ?ã×vŒ#d^?íu–Ob=ã?čsñidH¿æIÅ$½ú¿æ—:yx'â¿æ™Umß¿ÌD87SÿUNASNone?ノ¨]Å?³.[V-'?€]•ú$©?³.[V-'?æ¾ïÀ}ð,?ʄ½ÝyJø?҂ ¨?ʄ½ÝyJø?îʱ æ-á?—_"vã¼F?£Tåô0Öò?—_"vã¼F?èYDFxVË?®›ƒOf€Ï?Κîæ¤Ó?®›ƒOf€Ï?ï>£‰‡}¸?¢ÐT¢¶Ò#?˜+ŽÍXzû?¢ÐT¢¶Ò#?Ç—äkWš?Ìۏèîì?ê9Zå*?Ìۏèîì?ê}²5ë™?²oà ‡L?Æ	7+Qœ?²oà ‡L?¿\ÖtM†?ª©É¬P?ìe1vO?ª©É¬PMIXED4FGL J1724.5-3008¿°RÃâN†y@	aâs'?À:©¹¢MÀ;£­X"?
@Oe/Û@Á=¼#1?Ónä#Ösë?íÄÿxñƒe@zbœ­J?úbԘôF?ï^ mÿ¿Øꁺè¿áæ">iƒ¿ìªx^¶n¼¿ïÿÿ" 5•?á3Ê!Ì®oUNASNone?æœ^äx ^?Ð|ßí™~Ÿ?ÒÇB7¿C?Ð|ßí™~Ÿ?ÒQæ›Ä°ã?ɓ?gÒo?æ×²§Ž?ɓ?gÒo?ä5ʉð?²‡ªÒÔ?×ã"jìÄ?²‡ªÒÔ?ÓåÁ/µ¥>?²@àlë$w?æ
h%-a?²@àlë$w?ÑT&«²Ã?Ñ¥eaem?çUøìª&ž?Ñ¥eaem?•V¨¥€P?¢´GøjŸ?ïUJ»Ì-?¢´GøjŸ?ÁÓ¶\.:a?«‰wŽ\¼?ë‹hôqh?«‰wŽ\¼?•3yPÖ?€6ì>Ø;?27#?€6ì>Ø;	MIXED4FGL J1724.7-3737?¨Öåác¿ð¿Ï"èbUÀ9L‡?$>À:Îr«G@O²{<â4@YH;4Ž?ÎqUää?Þú™#R @
.9™~Á§@rx¨ˆIæ¿ïâ7,¼÷m?=î"2¿çù҉¥/пèsGà¿Gÿ¿ç!ßMØÑ¿ïÿè2_NUNASNone?í†ÿ V³?»–¥ïú_"?³ÈüáFê?»–¥ïú_"?æšt ý¡?ÇÆô2cÌÐ?ÒË¿Ô¾?ÇÆô2cÌÐ?è³
'k?°²~+¤Õ?Í3ׁöSž?°²~+¤Õ?ëX¥ù×Ðj?¥ew|Y
?h ¾Z?¥ew|Y
?é©è̇­‰?Ƃs•×uÑ?ÉX\ÍáIÜ?Ƃs•×uÑ?ĆkЙÇ"?Æô
­œÊ•?êÞeَ7?Æô
­œÊ•?à!ZŠ²mr?¸H'aŽPÀ?ß½Jê›%?¸H'aŽPÀ?ÇÿCå+?¶4X
$"-?ê/ ¹5?¶4X
$"-
MIXED4FGL J1725.1-1924?èwj¼SG@"ˆP›ùÆÀ9Oç"!°TÀ;‹M@$³>@FíùXŒ@_ž£Ä•Ç?½uQçÿƒ?Ê⬩@3ٛè(s@@~æ?ïýüºÑ!Æ¿á'Ñß^¿â7Š`@²x¿äè‰÷e&Ë¿î鱿«&4?ÚD¾@BoUNASNone?䀣b‰ü²?Ñð­&¿?Öþ¹:ì›?Ñð­&¿?ç¸ÁMÎÑ?ɏd˜9?Ў}db]Ì?ɏd˜9?êu^ÍÁ?«.l•x¤a?Æ+…Ê"Èý?«.l•x¤a?è¸ä.?ë?ª\QtÓ&?Ío"GV?ª\QtÓ&?ыXïìrÁ?É¢e'x_…?ç:Sˆ	Æ ?É¢e'x_…?À4¢ã´Ê?ǜl1×h‡?ëò×GýÍ?ǜl1×h‡?ÙôŒH<?¹E• é"§?ãr¹Ûáñ?¹E• é"§?ζœñ?³=˜ŽÛT?è{;{'XÄ?³=˜ŽÛTMIXED4FGL J1725.5+0840?í\}V9iû@7t>–=ÅÀ:8"ïïÄÀ;ø³ÓÃt@o‡]s@®^L¼q?Âv'ƒzÉJ?·4—¡Ç»k?ðÃmrÊ!ø?ûF°¨ÿ¾¿æáÀå7ý¿ß©jÝn…š¿ë¢†ÝÕ2Í¿àÀœ2#i¿ïýR¦–_¿ÝŠºC2YÄUNASNone?ïÊú"ô,ý?{×;Ë/?z'¶?{×;Ë/?îÀjL`<?¬ØlZtªG?£ù[9 Wð?¬ØlZtªG?îîÙ_m=?•œ5'mŒ\?¡j|á%?•œ5'mŒ\?îÜßÇ	?‡g4RÔŒ?¢2¥G=O?‡g4RÔŒ?î#êûáã4?«˜O$|øS?­ÁP>r0¾?«˜O$|øS?èG×ïYƒn?Í
6¨!Œ?Îà B™òI?Í
6¨!Œ?íÂT±2<"?¢²K7Ô:?±íZwJe?¢²K7Ô:?åõ'ª?¸ñùø)?Ô±ûî«ø?¸ñùø)AGN4FGL J1726.2-2903?ë«ô«õ"@'cj2¤À:3±6nQÀ;x'æÏ­R@Œz@ÎÀ§¨?ÒD@ ×f?ܺé"Ä@	Yšäó4@e
˜ÄÝj?ﶋ!±«‰¿äÑï¡c¿ÁáBWC¿äµüŸ|2¿ïýX «Ó¿ì òʍWUNASNone?îÿGÀ«N?±K£'¬§?®ƒd%?±K£'¬§?éGçî™Ù¹?ÁŒF¡òP?Êà`E˜™?ÁŒF¡òP?êž=Óá¥?©"ûÛ&?Ňˆ°yk?©"ûÛ&?ë[¯&&bô?¡ÑÐJcY?'Cgft1?¡ÑÐJcY?ê{‡Ÿ4ýÒ?Äæ«:€Ú[?Æáƒ,¶?Äæ«:€Ú[?͙£
¢?É.áÆ?P3?虏W:=W?É.áÆ?P3?Þ­Å6-?»*UéìmQ?à©rdûé?»*UéìmQ?Õ$œñà$?´r,¾&?åmô±‡î?´r,¾&MIXED4FGL J1726.7-3930¿î·Ïæq–ÀVq¬ÆaÀ9ÔÙb…UÀ;>"à4ê@>=I·™@¶
~C›?ÑkøvžÂÎ?×(Õ_°@Œq'êS@ØéÆW½¬¿îo<c]j?ïÓpöa7¿åƞµbLü¿èÕ·UlC¿æ¶9­ ·›¿éàbiªUNASNone?ïìŸo¾Ì%?d:ÄÜu?c`$W"©?d:ÄÜu?ï"ú;h?¡èÙ¿×t?› ¸ .®ö?¡èÙ¿×t?î‹ÈSI?œ¶C|	C~?®wC}_$ž?œ¶C|	C~?ï$1ÛoQò?'!]ÙR?›yē͏±?'!]ÙR?ï@Ԍg_"?™ŸÍ€ÊíY?—ånx;w'?™ŸÍ€ÊíY?駛ž#?Ì6 $…?Éc'‡sÊ?Ì6 $…?覟²@=?²gUq†?Íe6ÿÏ?²gUq†?æÌQZX?»®±·PAj?Ògã]KÏP?»®±·PAjAGN4FGL J1726.8-2659?ÓjçÛع@$ý£.mÒÀ9º`@²w·À;_œÈù@Bm¬@<eü´%?È÷ùñÉ?¶éÀ£s¸	?ós̀v²å@ýb–Î
?ïÿr ®Ì1¿Ý§š
\à¿ë'ÑÀ§zƒ¿Ùµ'm¿è1B}Sö¿ïÿÿ&¦³UNASNone?æŠ>7ѱ?Üh‰R"?Ò냐\Õ?Üh‰R"?<)&?",ì[Ù%¾?‡Uqtêé?",ì[Ù%¾?îµ³gd×à?šogGá
ß?¤¤É‰²'?šogGá
ß?ïÍ»io|²?^#ó½åóÌ?y"Ki=æÕ?^#ó½åóÌ?ïwæ	?¥ÃˆM¾e0?'n&¢vÐ?¥ÃˆM¾e0?íƒå¨:ò?¼òSgl?³àÒ¼p¡7?¼òSgl?ìÙ>O›ô"?©PÓ	_"?¹6
Ö€ì?©PÓ	_"?îR'Óê´{?—kÇÌë?ªÝ'Â0ŸW?—kÇÌëAGN4FGL J1727.4+0326?ÝGn=B'@4:GýœÀ:5N`¶#=À<§Š$Ô@˜ŸBÐà@ —ºœH¡?ÄOI¿;¿Ÿ?њIâøc@V1µ"±«?ùÝ£í¥¬¿ïÿÿ>¹ú?ïÿúŒ—Ó¿ÕÜýë©¿è€#¦Î6¿ã(Hr_™¿ïöÈHٍ¥UNASNone?îæAÚã2a?¥r0ç,A?¡›âR¨Àê?¥r0ç,A?ãC¦":i?Í#Ō¼'k?Ùx²×‹Ë-?Í#Ō¼'k?í·ÏBG+?¡L†L}	«?²A‡Åߪ?¡L†L}	«?è;Â"¹=?ª5M:—V?Ï÷ßu
?ª5M:—V?ꖒþõ¾Þ?½ðj$¥Àˆ?Å¥´)†?½ðj$¥Àˆ?Æò)A†¢?És,ZÚt´?êzƒu¯žX?És,ZÚt´?èØ N:\?³YþâQL?ͼŸ~Ç'?³YþâQL?̂ǐLé¾?³}»d?èßNìő?³}»dMIXED4FGL J1727.6-2304¿î3=͞Œ@37ÿJÎZÀ9O¹ã»ü›À;O¹ïzv¿@åªi @hLŸëÃ2?¿šâÑF?Â½é:ø@€¬:†
Ì?ÿ¥ì©&¥?ïò'íÓ­'¿ç5÷¼d ¿âµ{A¿½ñ¿ä} ½ê¿ãG ñO´¿ïü&Å¢·UNASNone2FGL J1727.8-2308?o"Äó?™ü'¬?‡ß¤>-û?™ü'¬?êDWz\´Ù?ÄfÝܶò?Æ,›?ÄfÝܶò?î;p¹¦[?Ÿ_¶zÏÏ?¬HôiãG?Ÿ_¶zÏÏ?ëfÌ4Ìet? Â'ßØh?ÂdÏ,Îj1? Â'ßØh?èf½Ø×áÃ?Åñ?yMÚå?Îeœ xö?Åñ?yMÚå?Ò*›Aü?ÑÂ?㓰?æê²_}ø?ÑÂ?㓰?ènDpE?·jÇlb???ÏÒFî?Òî?·jÇlb???×ÉÀG8	?µ§:äO?äÜqãü?µ§:äOMIXED4FGL J1727.6-0849¿é›Ð·×¶ú@,LÃ\á'fÀ:=LÖrgüÀ;€S`'@ø%ËÁ‰ù@£Ho›?ã/`•Áô?âræ§if@
D7'MLº?ýÔ(ì]`Ù?î'—L¸?¿Óx™q¤ˆ¿åëi~J‰¿çžb¿ïûh÷:^¡¿íòá~µ'žUNASNone3FGL J1729.9-0859?è]>Xžo?Ë{Lj?΋Ÿ½†D?Ë{Lj?ҌÝÅ(Ͼ?ʲ°"ê]#?湑k˜!?ʲ°"ê]#?êhÂ1pîÞ?©'mj˜'?Æ\÷:<D‡?©'mj˜'?ØV¤6«¸?³`c""W?ãÔ­äª9$?³`c""W?×6s©ç?Ð&O~?ädÆ+{Œq?Ð&O~?¥u·¶;ñ?ºø£>"?"·½Ð?ºø£>"?ÚÀò'iZ?¶nŒ ÛÙå?⟆ìKuÓ?¶nŒ ÛÙå?–'ˆóéx'?…<ÈXà?ïK븗­þ?…<ÈXàMIXED4FGL J1727.7-3621?ﺢ/ë*0¿êƒ©8sÀ8éXjËPÀ:6&æô–?@ 2¡'âE@j r}Ì?ù2«¹VÎC?Ô2k€³š@fî0Ê£'@ÜW·L?ïþÝ@7}›?Í.-ºÎG¡¿è¹]"?•A¿äÀåÙ
Lð¿ïÎ¿ìº?äŒt¸8ÁUNASNone?Ýz
'Ö?Õ¯U»üÎ{?áBú¶"üý?Õ¯U»üÎ{?åq¡&šN?ÑP¤c³>í?Õ½²Êåc?ÑP¤c³>í?áÅÛ¸¼¹H?·˜.&ÝN?ÜtHŽ†p?·˜.&ÝN?ç	¦}5hu?¾>Ê|K¼?Ñ쳕/?¾>Ê|K¼?áPX&Ôøb?ÔÀ7${×´?Ý_O²V<?ÔÀ7${×´?Ì 2÷=?ЋÔc]â"?èû·ûsB1?ЋÔc]â"?ÚzP¥×7?·v>?%»Ä?âÂ×­d€?·v>?%»Ä?°|[Äڌ"?®úÖƒˆ?íðt‡;s?®úÖƒˆMIXED4FGL J1727.7-4041¿ê_Kg¡>À	ë9\B 6À:B–Ù˸ÑÀ;Š¶ÂŸLa@'KåÓª@yX`ê%£?ȈH8}õÏ?§[Õ=߉"?ãè"=ƒH@2Âô†Ð?Óì{¿¿éòH‡XNv¿èÁ'ïV¿å'ˆ˜ÀUÆ¿è"Æ@–ž?º3˜ôUNASNone?ïôj1)Ì?\òcé>s?WÁ+:·¨ ?\òcé>s?ïÈsÈéW6?‰¿÷ÃSö?{ÆzÖE'?‰¿÷ÃSö?ï¤$EôE?ƒâV59Y?†þ¶ç£¶Ö?ƒâV59Y?ïàKZÇ?UÑM¿."?oùåñX`?UÑM¿."?ïÐ6Á)¢Þ?{ªŠFÜ-¡?wäŸiÌÿ?{ªŠFÜ-¡?GmÅ?³Ì[2€:?¤ÅëŽÝ<¬?³Ì[2€:?î‹"l<?œ«ñaŸ?§MߨcåA?œ«ñaŸ?îÇK*m3W?"xrZúó2?£‹MZ±–?"xrZúó2AGN4FGL J1728.0-3550?îV:ŠH ‰¿âÅuà¬ÓˆÀ8]qHA¸1À9óÍêÙþ@,³ô8Ìz@‰µ/ê©?ǃԠ֤½?Ù°ì1"@ªàéºC?ý­¼ÌN¢¥?ïùÐfqN¿Û™¨G²F9¿ãpöBˆ¿éÌòŒyöf¿ídÚu+ü¿Õ£ãßãÕÓUNASNone?åe=V£?Ó˜ÿjÙ¾?Õ5õ…R»?Ó˜ÿjÙ¾?Õ…³U#ë?ÌSËEÛxÙ?å½&Un
?ÌSËEÛxÙ?ÞwKõæ\?¶þöuÕ©œ?àÄZ·Ò?¶þöuÕ©œ?Ör·ã0¼`?²_ÏAo'?äƤg¡Ð?²_ÏAo'?Ò
zsÛç>?Ô±-ó5õ¹?æùBÆa?Ô±-ó5õ¹?£f·ðÌÐ6?²"ûƒ.?îɔñm?²"ûƒ.?¼–Š1q½?¨yøíÑ¥?ìm>.¹ÑÈ?¨yøíÑ¥?…|'*m'?vûäŒæé"?ïª
·›É?vûäŒæé"MIXED4FGL J1728.8-5131?ï_ ªº~À"\ú¬ÙèÀ:•:a%À;ñ3eˆ@'hC¶86@¯n'"šV?Ũ%$&Ñ?ƒEÍê"Ò?ÀÇ?EvW?ÿfwM"]p?ïCE.Þ9Ý¿è¼ýÇ%C¿æì€üê¡Ê¿å)	
Å»a¿à[BEÈa¿Û|M"ȁäUNASNone?ïù´M
[	?<œ$a@?I.Ë1à@?<œ$a@?ïä']œ#ž?wv˜ôgJ?kn¢S^BG?wv˜ôgJ?ïÞòA‡<?pm-iíqï?p†À_<aÁ?pm-iíqï?ïô{q²Â,?=[k¸P˧?W	M"hh?=[k¸P˧?ïñ¬§W67?RæuÃ:?\¦°Ûa‹?RæuÃ:?ïz=DØ‡?¥ÜÞÉ_Á?¸WhÕS?¥ÜÞÉ_Á?ï¸`4%Õ?'¤×éø?çóAL×?'¤×éø?利ëZM÷?v…t9àæÓ?†…0KºM?v…t9àæÓAGN4FGL J1729.0+6103¿àVÐ;
¿~@@³¥ 8LÀ;H!ÔfBÀ<•>zW@moe©P@³ê-/ãó?ÕÈ˒:*?Њ+<™¹O?÷åþFÂ\1@	0=Wyc™¿êë?{@¿èb¼Õ"p¿ãÊHŽK¿èìóþê×$¿ïÕ»Ÿíq¿ðUNASNone?ïù»üR?Cù"L‹Û?IÉðo?Cù"L‹Û?ïóÜ9ëøÑ?Y€ñ˜Ì?XGŒЎz?Y€ñ˜Ì?ï"Ï€¹×Z?'íKHƒ÷y?‹ßH™Z?'íKHƒ÷y?ïéÏ£'7?O|"÷>Ø»?f0\Çі?O|"÷>Ø»?ïøª¥ýÍm?M'UþTÓ?MUg"þ8?M'UþTÓ?ïÒtïÜ?xýë©_ù?vÅô
©ñá?xýë©_ù?ïPHGÊøj?ÜX:fž¿?•ö÷1VÈ?ÜX:fž¿?0<î?áv³üÌ?ßóæ¯0Œ?áv³üÌAGN4FGL J1729.1-3503?Ý‹pa¿Õ_/:€.À8Ý6ñLÀ:XoÌW@Š
Zvï@QÛèº?Ç¥ÿX:?Õûò•í=@Ç7ƒ$O@ƒê÷Ûj?çÀ;Yrb?Ô¹¥¨›•¿âŠèü®<¿ÞÛ	í¿Œ¿ïk›Äí{¿ðUNASNone?È¡#ï¦ôÿ?Í=£*"N›?é×·BÀ?Í=£*"N›?Û%£‰m¸¦?ËïÇÃÎvp?âm.;I#­?ËïÇÃÎvp?ÚÏP\†50?´«¨è¾†=?â˜WѼåh?´«¨è¾†=?âÚ«º®g1?³|€~?ÚJ¨Š£1ž?³|€~?ÐÜⶐlÂ?֗ÊE¢»E?瑎¤·ÉŸ?֗ÊE¢»E?«¸xÞ·Q?¶ÞòX~o'?îNÔxV—«?¶ÞòX~o'?¸Ë¯´Ù©?¦¢Žs–gÅ?ìæŠ	r‰N?¦¢Žs–gÅ?±oX-yÇ?›IÎÆ]X?íÒ´úPÇ?›IÎÆ]XMIXED4FGL J1729.2-2509?Ô-Ÿd@^øÀ9â"Óa;"À;3Ï`ûÃ@!/z–õ@uýfȌ?Õ6»©?å)Á¿þ]>@CEÎ@j?û_ò+V?ïÿTsõ›"¿ádpݸ­[¿æ}Kà~/†¿ë™ðlF¿ìV¯°¿ïÿÿ)@k*UNASNone?ç&~¡ñã?Ñ*çs°ëŠ?ѳ¼ü:?Ñ*çs°ëŠ?ÈÀ×&©V?ÄþS¹'?éÏÊ6U¸ª?ÄþS¹'?çÀ?:¨rz?°®kï¯?ЁŠ¯?°®kï¯?ÐÑ_`ì?°N}ʚ¾?ç—rvPOŠ?°N}ʚ¾?æ+kyÜÌ?ÐüII?ÓÍ©)Fh?ÐüII?"ÒZÃT"æ?ª^&½ø?ïYm)םi?ª^&½ø?؟6	/[?µo1~6Ê?ã°dûh|Ò?µo1~6Ê?†5'q"?vj÷wZ?ï§*'9\?vj÷wZMIXED4FGL J1729.4-2831?îŽ0Ä1âj@	È*ÜLœ'À9¸ª½®KØÀ;_ÐJ/Ï@-ò»ô¸N@m.#(ú?ϝúé×?âÛÛÈé~@‰Æ×p•?óëà;§R?ïÐ•¯)N¿ÙsÇwù5á¿æ(oÀ';¯¿ì6ĸ+U¿æÑôSúS¿ïäîâKd,UNASNone3FGL J1729.5-2824?ëRhU‡y?ÈÈ5°³^?¶^©âÄ?ÈÈ5°³^?Ìw"ª$3ï?Å:"¹q?èâÕvó?Å:"¹q?èQ…§?±"š@?Ϛ¹‰ùéf?±"š@?Ö'§†8¶?³ØKDYȵ?ä÷l,<ã¥?³ØKDYȵ?鷄m&bÚ?Ì(@#d;Ç?É!îKft˜?Ì(@#d;Ç?"¶êT ã?¡7I0_>5?ïbH­vxá?¡7I0_>5?܃DʊR?»R€ç'@ô?á¾s]šº×?»R€ç'@ô?ŠR@ÁRñ?ƒR´X8݋?ÿlB…?ƒR´X8݋MIXED4FGL J1729.4-2646¿ÊqNnDx¢@¬¨ââ¸ÇÀ:`{l‡è—À;ˆÌ&°n@û8|É)T?öœøä'Ëø?ç§"ïQ0?꡵A•Ì…@Ãà{Ö:?üôRÝÊ?ïÿð懈ö¿ë$¦=¿…ãÑZÞ¿å_ú†C{¿ïÿŸB%‹¿ïh‹9"†UNASNone?êҝºÌ«P?ÈýÎÚ:•õ?ĵ‰ÍRÀ?ÈýÎÚ:•õ?䈵¾"N&?Ï÷"Û`—?ÖÙc´?Ï÷"Û`—?ç)8•j,f?®ŽìcãK·?Ñ­ŽÕ+§4?®ŽìcãK·?ê|z¯#J?ªH{Ý°šž?ÆC«r×?ªH{Ý°šž?êÝ1
±VF?Ìå™	ÚQù?ċ;Õ:¦ç?Ìå™	ÚQù?ÄÔÿ/d`l?Ìq]¼@/?êÊÀ4&çå?Ìq]¼@/?ރhdîA<?´Êð–"?à¾K͈ßb?´Êð–"?ßMQØ?Á®?zá"ý?àYW@ýt?Á®?zá"ýMIXED4FGL J1729.7-4242?ß4ÂcÙÀ–Â&€IÀ:71xH:À;£¨z-@&‰/=õ@Q¨òÓ?ÔòI~N9Ÿ?äh¿µ<@‰å\ËO@íõ!È}?íD¹ØÔB?׸ÎG*a¿æœ†é"¬ñ¿é‹@•¿ïKtÝøn;¿îÁ†b…0VUNASNone?ëEPiyì*?ÅÖ.0¦!N?Âê¾ZOW?ÅÖ.0¦!N?â…ýÅ_'"?Ï6œßŸ7h?Úôu@Úø?Ï6œßŸ7h?é9h®!â?¯«âæLw=?Ë]Góxw?¯«âæLw=?ã»gäY ?³®EëJ%?Ù؉07LÀ?³®EëJ%?æC† &LV?Ðô‡èRu?Óxó¿³gT?Ðô‡èRu?À¾í}¾¿?ÇT^ډ?ëÐD P<?ÇT^ډ?ÖÐ<'€ ?¸ð9&ƒ?ä—áìw?°?¸ð9&ƒ?§–:öhU?–\u†EÓ?PÐto?–\u†EÓMIXED4FGL J1729.9-4148¿Ð¯9.òBÀºG²À9t(<æÀ;g
"fy²@àn"0žÙ@՟Ú%{?Àu	l?·uPdˆr?ñ>³nW@Ç'¹ØSi¿ï·б]Û?ïÿ´Jõǘ¿ækÑ	ro‰¿æ'á>sÙ¿ànw¬ßÇ¿íBåøí½UNASNone1FGL J1729.8-4148?ïë!«:D¹?˜X‹Æíñ¨?dÞTéw6?˜X‹Æíñ¨?ï×À|˜"?F–Aè.?tÁ›©.Ü?F–Aè.?ï‡?\êÅ9?ŠÝ(Poä?Ž0(ÁßÌ?ŠÝ(Poä?ïÜePç¤?]\šˆH´?qÍWwNO?]\šˆH´?ïÛ
Ÿ›×?rùðžo‹Ž?rz°/",¡?rùðžo‹Ž?îÕ¼‹Íp?³z~Öq?¢¤7KS?³z~Öq?î\·Q¡™~?¢
ÆhÀÄè?ª4ŠâvÌ?¢
ÆhÀÄè?îñ54Ƚ&?"ÎN÷"? ì¬¶ãɗ?"ÎN÷"AGN4FGL J1730.1-4343?ï'¨æiÀ[ÞM'ÑÀ:.¼ÆÅKÏÀ;¡=ȸk@ª|ÂqU@S°ÄXŠ?Ñ°™É=v?é(¶!å'ü@^(}ˆÂ@¸¢kOYZ?è–Dzƒ?í`ov°`…¿åú´f¤z¿ïý»aëW|¿ïí¼ '+"?ïƒnI‰¶ÎUNASNone?èä
h[*•?ÊÐj!›S?ÌoÖ^"Uª?ÊÐj!›S?â
³"8ÿ?ÎíSY]-F?Ûûä˜×Ž?ÎíSY]-F?çö®H/ø?°3,á·ù?Уo Ä?°3,á·ù?ãòô=»3?¶TÌöe?ØÆ"‰›?¶TÌöe?ß.¤óø'?Ò71ÑD'ç?àh­À¿?Ò71ÑD'ç?¶õy¦¸z«?Âjâí¨'?í!PËR+ú?Âjâí¨'?ÑÌܒ»?´"'ñ«a??çx™'¶÷#?´"'ñ«a??¨ÍêÇ3Ò?˜è	B'ž?îs!Srÿã?˜è	B'žMIXED4FGL J1730.3-2913?ïzÒ>Ú8ú@Z¡ô±îÀ:Àk<ŽüˆÀ<Y<Íù@Ã÷h+ã^?ÿ{xFbºà?Ö·Tà¬þ{?ïÿp=½P@¶WuÇ,@‰-Vû9r¿ïa.ƒ¡	Ð?ïì­"šB?¨o‹þüIè¿Ó¼_vÞ¿ïÿÿ>¹ú?ï߯BxJ"UNASNone?å6yÖI'?Ð˲
o™?ՓõSlÜ?Ð˲
o™?èæççÊ?ǹ݋$Љ?Ìd``ןþ?ǹ݋$Љ?çŠ]êÖ?±oÕƒâ?ÐëD+ÓîT?±oÕƒâ?é¦d\º°?±e+µ‡Ù?ÉgênA?±e+µ‡Ù?ãᢺ»¹?Òi B*Fû?Ø=ÔºŠˆ?Òi B*Fû?ËÍXҘØm?ÌÚ¿Oqéc?é©ËYÉå?ÌÚ¿Oqéc?ڏ
þF?¼U$
•-¾?â¸~zôÝ?¼U$
•-¾?Ôn/ˆƒÇ ?½ë~—úKû?åÈè;¾0?½ë~—úKûMIXED4FGL J1730.4-0359?ä-íaþÞÔ@/ý™gD²·À9¡ƒJ¢»À<	²öañ@ûŸZMÔI?þ´zuçãª?À_©]ÜÕ?áp'S­Q@B¸A$~?ô˜0m±v¿ï´qV"q?ïÿÔač¿Ãݨè)b¿æ¶ã¡¥¯¿ì´/GhG¿ïÿûÞ]BüUNASNone3FGL J1730.6-0357?Š`ôùØ?›ò¡3)_?ï—â|Xãh?›ò¡3)_?±·ñŸ?³Ed½›Œ?íÉ,&_Ì?³Ed½›Œ?ºUChài7?¥Ä[~ÊÄ?ìµW'ãòÙ?¥Ä[~ÊÄ?"Ü.qi??|Ùÿ´ÔÔ?ïazö?|Ùÿ´ÔÔ?®­ôÑ?¯1tr;Þ]?ï¹G•'"?¯1tr;Þ]?Š‰Hv?•»À*À"?Ûéw?•»À*À"?¥õç[?~C²ÑˆÒ,?ïh(™k?~C²ÑˆÒ,?E'ÄààL?:|®_g>?ïú›Nûe¼?:|®_g>PSR4FGL J1730.5+6018?×ñ v'"C@@¡êhìSÀ:ǀõ]åŽÀ<g;.ª7@:ê¡tˆ@øåY‹?Ì<"1/?Ç£&
UÄX?ùÐéÅ@X—)§Ä*?àℏFY¿ÏRôčŽ¿éo6žø~+¿ãWB\	¿î{bâMg'¿ðUNASNone?ïސ½Òß?pњ#C²K?pü·˜'"?pњ#C²K?ïàS1Ó?q¥:s+¹G?oî¬ÒЬ´?q¥:s+¹G?ï ¹)hx?€IÔí¨ž?‡Ñµ©j~?€IÔí¨ž?ïtðš‡UI?p¦×t}?'aì¯VÔ?p¦×t}?ïÅ'*Ö? ¤tô:¿?œ§[Ì©/? ¤tô:¿?ï|ºT"ïÐ?'R^Hj?hµpñ¡ò?'R^Hj?î$#€¯? =VˆÞòz?­½Çø÷? =VˆÞòz?ì8iìC$? â-\.ª
?¾<·æä? â-\.ª
AGN4FGL J1730.8-3806?Óäÿk÷~À'¢&0À:@[9âzÀ;šÒרÈâ@LR_žK/@@þ¥Œìã?Ñcêöƒ|?㎻ßê‹Ð@ÊeI/ôº@AæŽÿf?Äöë¿Ý—Š ­_¿Ô«ÉGNÏ¿ãÀ'¢Ü8¿í"rmÛ¥®¿Ý#ÌbïŽnUNASNone?Ü¢E®Ï¥‰?Êúd{Ö8?á®Ý(˜-<?Êúd{Ö8?åÄäÏx?Èe«ˆWä?Õüwà6a?Èe«ˆWä?á9D1k¢?³áÛ
ìÜÑ?ݍwï(½?³áÛ
ìÜÑ?è²79t?¦šñЕÃÇ?Í7ó#-Ë?¦šñЕÃÇ?ÁÝܶòw?¿y®—­†6?눈ÒC{¢?¿y®—­†6?¼PC(7›g?Â
2U_$?ìu÷šù"?Â
2U_$?½uï¨;j\?¦ÉnÌÐù?ìQB
ø'µ?¦ÉnÌÐù?Ê(¹S´?«nä¬jì?éuýѸ«?«nä¬jìMIXED4FGL J1730.8-1123?émËxÉQ@(EºÓ¦âÀ:´Ÿèh3ÆÀ<†íÅjÙ@!OµX«h?ú‡ºt´›?ÕD[å$x?ÎJ>ýìªc?ñL <K	ê?ÿvà.~m™¿ìhûl‰?ïø ÅÝÅC¿æN'à¿±kØ@Ho…¿ä¸
¾
¿Ùj"‡0áIUNASNone?ïíÁ¬ˆ3Á?aÊíQ‡ü?b>S5Ó¿º?aÊíQ‡ü?ï@þD›?§nµé|?—à?ÒE5(?§nµé|?Vä¤k?‡}"cr-S?jT•U(?‡}"cr-S?›¸,Ø?o¼…ÃØH?ˆÒ³:?o¼…ÃØH?ïáÂ
Y¨Æ?p÷Žý£)?n=õ±Uù‹?p÷Žý£)?ë‹~?îNõ?ÅyŒw¶ß"?ÁÒFÄ,?ÅyŒw¶ß"?`µfC? 'ol•?§•9ð^Ü? 'ol•?î>FJÝ)?žRz¦XQ¢?¬›Zò'n?žRz¦XQ¢AGN4FGL J1731.6-2904?ïÐ謹@("[CóuÀ:Î.äðÀ;cä|캩@".çßCr?ÿ´o"͊b?ÇB]Þ¨w?£©Þ
aظ?à¹¡Kê?ûë¹Èä
¿ïø…'‹`?ïÍ/(·Ä¿Ä û¸•Ó¿¸Ôç"ŽuN¿æ)S¶`y½¿Ñ'ó—»HUNASNone?ïû Ðg?qȍwø4/?Cå}x5;%?qȍwø4/?ïž÷< ?—¿
zª)?ˆxB*À?—¿
zª)?	"žû?‡¹F_Ø?‰Qý¡÷y-?‡¹F_Ø?ïª:÷«PY?t}A!ð?…qB¼MË?t}A!ð?ïúèoÍ?O¢I"óó,?D_¢QJÌ?O¢I"óó,?í>úž'÷?À¸É÷¹F?¶+ šÇ?À¸É÷¹F?î²ÃxTl?œùeõâ
?¤ÓÈ{š°9?œùeõâ
?î—–×iÖ?£Í­1!?¯Ö†•š?£Í­1!AGN4FGL J1731.6+0630¿É×5]§Gz@4®IäO QÀ:ç¦3ÛϟÀ<oyÌz@§5ÐòKa@)¹à<?×ê6jX‹?ïÿæՌŽï@zy5v'@Pԏä¹þ?ëŒÜ­¡¿Ã;—Æ/Ϧ¿ê
@?‹0J¿ïÿCwN7¿ïäÚ_²m%?ïâiamƒ;UNASNone?î&¼`,í?¶É2ô=÷?­"9üX´*?¶É2ô=÷?ç•qݤº?ÌZ[k5®
?ÐÕD·ÈŒ?ÌZ[k5®
?ë[ž¨2tÙ?§ú¨îšS³?'…_6,ž?§ú¨îšS³?ége@ça?¯»>û€xè?Êbjÿäb|?¯»>û€xè?ìQî‡)!?ÃÒææ%õ?½wx‹Æ¶ø?ÃÒææ%õ?ÀPûÒì?Æȅ¯?ëëÁDùü?Æȅ¯?æPWü?´'á>sÙ?Ó_QÿÒÊ?´'á>sÙ?Å@!î'Df?³~;e`öÉ?ê¯÷"[nç?³~;e`öÉMIXED4FGL J1732.0-2659?ï÷ØÉQº@¨5ÞßÀ9£Y#‡Ä…À:2K@]':ØC#@ì=áò?ÐàƒãÏÈ«?É=+Úy]º@ðAFm@­¸#®?áµ "µ7?ïøŒ8ˆÊ¿à0rÄBº¿å?þÞ÷¿ß'Øa*'P¿ðUNASNone2FGL J1731.9-2703c?î|þz¼+?¸(Ì÷ÆÉÉ?®ˆ0ºS?¸(Ì÷ÆÉÉ?ébôˆõÔÐ?ÈSã¬ã"z?Êt-Ü(¬¿?ÈSã¬ã"z?ë·uèíóA?ªù'Û§‹>?Á"(\H2ý?ªù'Û§‹>?ì¡Ù,&?¡DE?ºñ7>ŸfÒ?¡DE?åñMÕB^—?˜Ý3—î?ÔdU{BÓ?˜Ý3—î?Ô8Ú*ó
?Òݒ~ ?åñã'ê†z?Òݒ~ ?â×<? |L?¹¬
Óv<Ñ?ÚQ‡¿g?¹¬
Óv<Ñ?ܗ¾®ã?ÀñÈmEÉ?á´ ¨Žvr?ÀñÈmEÉMIXED4FGL J1732.7-2559?á¾4Ô¦"†@ÞµÛ¿êÀ9Àg{9\BÀ;?÷ˆb9±@ÿ‡ý@k§áZùK?˗©jÄD?ÔÂfa³Ï%@
˽Tn?ùÔ«JF¿ïÙ˜f"³?ïþáòο¿äjd!舿æð,µÿ+¿ì®a&ák¿ïþŽ`€sXUNASNone?êâ"6-0?Æ%ò­ÜòŠ?Äww'K?ç?Æ%ò­ÜòŠ?ÑôÆÅw?ÈûÕß?ç…œÀE?ÈûÕß?翝	™9€?¯Ô35v?ЀÅì͍?¯Ô35v?à[uÊ»S?²£"Z,«¶?ßIj‰û[?²£"Z,«¶?áï[J(˜%?Ð ‰ž‹7?Ü!Ik®Ï·?Ð ‰ž‹7?œmä¬d?°û–ãi˜á?ïß¶´]?°û–ãi˜á?ѳ¢ëc!?µ+¶aË?çx&.ŠNo?µ+¶aË?©0ælz	ƒ?šß[¦·?îlñ™FØ?šß[¦·MIXED4FGL J1733.2-2915?暑…lL@@öÿÁßeÀ9(=5ëtÀ:}äÎv@ƒYdJWg@"šVWû?˱AÖäþ?Î^® º4Å@Xùã†M@èîüwŠP?éµâ¥|%ë¿ãu
¸A%¿æîZY‡¿æ@å£]h¿éßb"Ò¿ìu¦à©ùcUNASNone2FGL J1733.2-2913c?ëîBpñba?ōŒÌgÞG?ÀFö<:v|?ōŒÌgÞG?ì­%€JÆ«?¹½îæ?º–Óý©Ê¥?¹½îæ?ç='ªŸ?´ÇÙ>'e\?ÑDŽګîÂ?´ÇÙ>'e\?í߅-ž?šdE<Ã,?³÷ÙÅ?šdE<Ã,?껪'Ÿ¶O?Ä2)æk?ÅU¹&Â?Ä2)æk?à !.?Ò$€{\å?ß¿½ñ£×ò?Ò$€{\å?ܲœ†E]?¸xâ,ú?ᦱ¼ó]R?¸xâ,ú?ØJô•"¥?¾ëÑ	ro‰?ãڅµ6-9?¾ëÑ	ro‰MIXED4FGL J1733.4+2235¿Ù–^?•0@:²ÙßÚƋÀ;k¬ºÞ¿À=G€ß֕@d@ÚÖb@ÚÂXÖ?Ӂ:þϾ?ïÿ4~ô€@Ù>½ªðÚ?ýCw£ûrR¿ãHƒýP"?ÄYbFò?ïùíÎ à¿çdU/¿ïÿۂr5¨?ïüQ¿æ4}UNASNone?×Ik·Lø?Ð!>Í?ä[7Ê$Y"?Ð!>Í?ތ¦Äð™?Îõd^å?๬ò´?Îõd^å?âyð©BP?µµ·"I?Û­{_?µµ·"I?Ó%>I«‰?¹80'åø?æmtàÛ*;?¹80'åø?Á]Û?"Í?Ê
§#¶?먉07LÀ?Ê
§#¶?¶*ʔDb^?»n¥?í:¦­[öÔ?»n¥?Ë>&Z¡zþ?»òÑvÞ6_?é0viW¡@?»òÑvÞ6_?®eubž)?§q¨è*Ç?îù¨€šÎ?§q¨è*ÇMIXED4FGL J1733.5-2950?î|mÌÄÎ?û»gšCÅÀ9–,­®À:í¡(TH@!;rò»Ê@âIC?ð±?ÊôþÑpË?¹6xð+Í?ô»k±)X@]¬Ùge¿ð?ïþ$É
$¬?ïö)óð¿äJN듿çÜÖÐ[͆¿Ã-ˆú:UUNASNone?ïè¦äÍ?‡ÇöyCÉ?gíY­@û~?‡ÇöyCÉ?ï'e®Î,?PdlGC?‹¦¿›+­?PdlGC?îRú´ø«ß? à'Sž;)?ªÐT­¦? à'Sž;)?ïSn•<›D?ˆZÖ¤â®ÿ?•'-V´Ét?ˆZÖ¤â®ÿ?ïÕL+bën?"<Eõ
xÛ?uYêFû%?"<Eõ
xÛ?íd+¢–?À-ê"2ýX?´Þ¢ñEÍÌ?À-ê"2ýX?ì7*Cþæ?°9©~oðÉ?¾F­àÏî?°9©~oðÉ?ìÛbPÏr¼?°ÂéhÄÃ?¹$íyò]¡?°ÂéhÄÃAGN4FGL J1733.6-2431¿æô=Te@hŽ^Òô.À9Õ]z.šGÀ;s‰½×g@0™@
ûÖ¥"£?Ëæá õ?á…X'@-+Ç.'?ýÑ}3'–¿ël{ž†é>?ïùÒSõJš¿ÛÆ~1ß ¿ç"ebZh+¿ì&îRz÷¿ïðx£ÌiUNASNone?Üú+ò™‡r?Ïð|8y‡ð?á'ê³<G?Ïð|8y‡ð?ɕÉ[å?F?č®ÎMð?隍©°/?č®ÎMð?൙Ü2·?³ÕBñ©?ޔÌxǚ'?³ÕBñ©?×ǐÎÕ÷ª?¯`ԉ¸-·?ä7˜•+?¯`ԉ¸-·?Ëí•ð?ËUTÈP³™?é?"šƒú?ËUTÈP³™?"R/Zˆ"(?§ëÿ€É×	?ïen…Tú??§ëÿ€É×	?¹e£åü?¤ö|Øõx]?ìÜýSt¾?¤ö|Øõx]?¡7MÿOFˆ?Ž?½×§ÌV?îì‹ &ˆw?Ž?½×§ÌVMIXED4FGL J1733.9-2220¿ÞeGÉSÃ@℁Ú`3À9Ÿ¬îàóËÀ;#J\D¤u@TÞ»·¦ @óà{Ö:?Ñ,à]Î<d?à€å7ýO@úuÚw°;?úÞÿI¡´›?ïÅÝÖ´¿ÜGm\¤Æž¿ê³Ãp=U¿íHzøÄ¢\¿ïÿþˆ0»Š?ïõÁ%y·UNASNone?ØòI_³«?ÒvÓªü1X?ã†ÛsP&+?ÒvÓªü1X?ț4 ø	?Äé`…•šu?éÙ2×ÿÁþ?Äé`…•šu?ç¯lÈ2è?°ÝàD0®	?Ñò¡&oš1?°ÝàD0®	?Ô½/ðLrŽ?³Ç«…gÕ?å¡hÙƹ?³Ç«…gÕ?ÌÆ°bÖ0?Ïvõ"æÜ?èÎz"çJt?Ïvõ"æÜ?Šý[M3?žZ0»p?ï—ð
®H—?žZ0»p?Ó£€@_Ê?¶¹…áð9?æ.?ßÐñ?¶¹…áð9?fÐÑ䘬?uƒ3Rr%¨?ïºd¼†ó>?uƒ3Rr%¨MIXED4FGL J1734.0-2933?ïÿïI#Št?üø[ÆÐ3ŠÀ:Jøš°ðÎÀ;ÿGóÐG@ ;<hfç@2Ú˓?ÖöÕ^ìŸ{?ï?CwN7@
º ¢¢V×?ýþ0Çóõ¿ïÿø="ßE?ïÿîÝÃÀ	¿Ú~ߟã5¿Ö¯£#Ûý¿ëtcˎ߿ï´ì`»×‡UNASNone?ç§Ät[?Ϧœy`W?аwIÙÏ?Ϧœy`W?ßWåóB
?Íê³tƒø?àT
^úó?Íê³tƒø?è15:' ß?±°=8qjä?Ï;+c|…?±°=8qjä?Û&ñí?¸kX—àu»?â|lÿv‡
?¸kX—àu»?ßÝ÷ӜÛÕ?Ò[VÂ`'?à1'?Ò[VÂ`'?·ÅÅΜ?¿º±"¬?íG^'A|?¿º±"¬?ÞMû¡	?¼$Õĺ|?àÙ~p¯|?¼$Õĺ|?«ªßŽ±¹?í
qôP?îN•RÓT?í
qôPMIXED4FGL J1734.5-2818?ÜnSƒw/@[»èxûÀ9yÂ=ägÀ:ô˜"¶Ü@F3#îǞ@N¶Ú@¨?ÊöíÈ
˜?纽֏Ä@ð«†+(@úfÛ×+Ë?ïl-_ߎ›¿†ÏÊ¸Ëc¿Û«n®3"'¿í*__6p¿ÚŠ|›1[¿ïûr»UNASNone?çèߎ+¸?Ìsó2ÎD­?Ñâ.@㨏?Ìsó2ÎD­?á³Ù$¸µØ?Í5\Sú`?ܘM¶Ž"O?Í5\Sú`?åsÖ¼e?²cÍêg?ÕñçR‡6?²cÍêg?ê}))?¬DÐdgûÀ?ÇûûÂ[[?¬DÐdgûÀ?Ú:Ó{Ä#?ÑýëqíG?ââ–Bwï?ÑýëqíG?«"¼Ù_à?³ˆit\½?îFÄ2}r?³ˆit\½?ÜÌÔY‰?½ØP0‹`?áÀ•Ó;|?½ØP0‹`?ʄ35˜¤?¼þú±7?é^ó;²™×?¼þú±7MIXED4FGL J1734.6-3548?ÞDX"6¿úýª…z'äÀ9Žœ÷+°À:זߪõâ@ /§zùª@bŸYÌúð?à•
ÞÖ9³?£N
ÿòê?ÙOGß=@ú±Â¸L?ï¼Ü)a"Z¿ìe€Y¿ä¡¿½ð÷¿ç8° œB@¿î½©CZÉ?à'F¿,%MUNASNone?ï/ctBŒ?¸M»Í/¥?šŸ¿à‡?¸M»Í/¥?ïҕÍmlÑ?‡>›Ç\þ?vµ1<S'?‡>›Ç\þ?í[KïÜ`,?£³³›Ì?µ% øå›?£³³›Ì?ïÜ`Z!£X?`"œ×%?qÏÒô­´'?`"œ×%?ï,E͔ž?¨ÍóùÊL?š}×?n4N?¨ÍóùÊL?îê?–më?±?ç̂z?¡V,uM?±?ç̂z?ìî­û®ë?¨9Ñ%)¸¿?»€Š"ˆ§?¨9Ñ%)¸¿?îšlÑ<æ?›Ë]ÕÖÞ4?¦Y2ñû͚?›Ë]ÕÖÞ4AGN4FGL J1734.6-2912?îŠ
ú-?þ2°ì©À9¯mO"¼À:À'\f2@!Jgö…`@`RP/?ÎË]k"?ª]TïÆw?åóø :G¥?ü‹Å~
¿ïW?íUÙP?î>3Æà¿ãí^½¥'v¿á*Vµï:¶¿àç'Áåèþ¿íõ¿4]ÖUNASNone?ïâœæ2×÷?Œ©q¸Zù?mc·àÓ?Œ©q¸Zù?ïP1^S?¢¼W?•þyÔ=•ž?¢¼W?ìÚi<_?¨›øŸ‡›õ?¹,¶õ?¨›øŸ‡›õ?ï"ûùqVÁ?yÌåàêÇý?ŠÁ™[{ê?yÌåàêÇý?ï̐c²Ni?Ž3õÕù?y·Î#i/§?Ž3õÕù?ëi"ÏcÀ?ǧr)'Z?ÂY¬Âsá?ǧr)'Z?ìCrp?°q²|)÷>?¿…çdlõ?°q²|)÷>?ëhjâ.M?µ»BC*þÛ?Â^W¨wFÍ?µ»BC*þÛAGN4FGL J1735.2-1640¿ïDF^ç @ ú_"ÊÕ|À:*M)~~‹À;ÏžÙt{@4¶Ë®"¨@ÔbÞ©ª?Äü"_öŠ¶?À'KÊ-á?ùôàM/^@½Ï®Ôi?°4íóc?ï-*ÛuÝ¿ãj'ñ¶'!¿äM'àAô—¿íh!Äuæ?ЧÍęw‹UNASNone?ï—^¹Háp?Œ\P"	j_?Š(Q´¦Ûä?Œ\P"	j_?îâ%êJa"?«ráwhg)?¡Ý¡^ɉØ?«ráwhg)?îdTNd?šÌô"N÷–?©¿¿k\½?šÌô"N÷–?ïtð(,Ö?©ôs‰?Qaúúe??©ôs‰?èWþƒ˜?œÐƒO*?ÍÊ£¬ñ ?œÐƒO*?å
|¨¥®®?й"dțT?Õå®´¢£?й"dțT?êӖ·pÅ?²mí¶œå?ı§"<ì?²mí¶œå?êSãQg¯?²0ur˜¯×?Æ°qŠºaC?²0ur˜¯×AGN4FGL J1735.3-0717?Â'¢xåÅ@*":귙_À9iݞ¬(À;l`Nq@2pÃa"@	ÿ&ò³?Á0/GÁ4¾?Ð0&£Ø·½@»)'<†@¼ƒ †]R?ïÞM}·:ê¿ßøQ{¿ä¥žŠš"V¿é+î›S­ý¿ãœ/vQ¿ïö¢¾ÜIBUNASNone?êm²öañ?¿ú
slDˆ?ÆI4&x9Î?¿ú
slDˆ?Ù-þqpÁÅ?Ì<`X…R?ãiÇGŸ?Ì<`X…R?ìÆØCÎ`÷?£
«Ò?¹É=áŒøL?£
«Ò?ä>	¬ëÊ®?¯SªÙ¨?׃ì¦(j¥?¯SªÙ¨?ÕÈ3¦Ü´]?Å'hƒÞ-?åæ,'¥Ò?Å'hƒÞ-?ªB"&ø\?ºÚÖb³æ?î[ÝÝ|ƒš?ºÚÖb³æ?â®bmÕ½Ú?µØúB?Ú£;$T"M?µØúB?±ç{x É?ž±ˆè`?õ?íÐÆâ'?ž±ˆè`?õMIXED4FGL J1736.1-3422¿è¼wÑ·‡¿ò¦J'ÛÀ8ϙ O–@À:ùÞØh'@üpí(@ÐÔ¦2.?¾ÝþMxX×?ߙrb+Š@:Zà÷&=?ÿ=«‰Ü[?ç¹`>.8ø¿áþÐW›È¿Ð•ŽÝ}ôø¿ââ7ùk'¿îõ"€-¿ïø¾nèìUNASNone?–Œ¶-åE³?£g±(Ò=A?ïKšNº"?£g±(Ò=A?À|="3xþ?·t}¯/p?ëàð›3!À?·t}¯/p?¸f·0b±A?¥‰Ž0EG?ìó)*£˜?¥‰Ž0EG?¿n $UÓO?¡³«Úã¶?ì+ûuE–?¡³«Úã¶?ŸFÙïÜ?¸Lã€í?ï½Ðè±?¸Lã€í?!Ÿ"×Ù]?'¨Ñ•Àc`?ï‹y‡eK?'¨Ñ•Àc`?û;0hä¬?•l'X?ï&&Áq
?•l'X?r)ÇBY™?`j]\͙z?ïÛ¬q–"õ?`j]\͙zPSR4FGL J1736.3-2929?îY(2N0å?ö¹ïô8À9'7›wÀ+À:¢êºô]5@ç+¶'"Ø@FºÜà@G?ÎUíQy?׺¾A@
†ðÝMM'@1•@C'¿ïÿíUÙPi?ïÿ¾ÇPŒ
¿äXeAxEa¿æړ)=,¿î{J#9Àì¿ïÿèþ†®/UNASNone?è@˜×°^5?ÌÒ¢?Á*?Îýœ¡>‡-?ÌÒ¢?Á*?àŽ±ò^ŠX?ÎF'Ýû¯u?ÞâœBëQ?ÎF'Ýû¯u?㎠p'(%?µ_†²¾#?Øâ¿Û¯¶?µ_†²¾#?æò«wMÐ?´&mÌ{!?Ò©d_?´&mÌ{!?ߒXM°P?Ñ1먍°á?à6ÓÙ'ñX?Ñ1먍°á?·t-"$ú$?ÀÁFSBêƒ?ízM›`»?ÀÁFSBêƒ?Ñ£Ò‹0S?µ‰Œèþ~?çp®ºg×?µ‰Œèþ~?µ??s?ª<—Ÿ";~?í_8Ú£`?ª<—Ÿ";~MIXED4FGL J1737.1-2901?æa×ÈJ8?ø†jGœvÄÀ9Ž™‹VáÀ:b4¡È<D@«šêÒqQ@!dԕï?Ё^ú·@É?ÓÛÊ@«kÔ@¯d9Ö@
7_½ªÆ?ìó0®ôt²¿èmÝ¿è̞
²¿âZ£"Ôæw¿ï鲀ñ,(¿çKù"k9àUNASNone?é0B›Žš?Ð#K·ÂJ?ËÏ>õ'Ř?Ð#K·ÂJ?ê55õÊ?Âý×ÂÛB˜?Ç+›((×Ô?Âý×ÂÛB˜?æ¼±\êù?´™$$ö¥%?ÓֆF*?´™$$ö¥%?ë«£J%Ê?¥¡eªy?ÁQr×k"×?¥¡eªy?ë³ËJ&ûÔ?Ã4®îQ?Á0Ò×d²?Ã4®îQ?Õÿ5!Af?ÐÂQd²ÃG?å}eo_M?ÐÂQd²ÃG?ÞøŒà‡?¸;û\@îi?àøƒ6½?¸;û\@îi?Í‹*k
•?µ³Ü‡à¥?è]5e<›?µ³Ü‡à¥MIXED4FGL J1737.2-2808?¦²Dó–?ÿÉåA7Ø´À96"S.{>À:Ž"%¼R@сd®M@ßdš?ÏËø&êþ?ÁB%©Ý´|?øXà66ò@²°ÈŠGí?ç
«NÍÃm?Ú#‰<TD%¿ì¼W3Ã{ë¿â¥¥@–É¿çÞÉ^®64¿ïÿø="ßEUNASNone?ï•JêVlì?žFM[jê?Š­Ex#5?žFM[jê?ïTÝÁ«u?¦|5µ'?ŸµdLñûN?¦|5µ'?꾒G‹&?°9ЖÐ?Å·†áÓg?°9ЖÐ?ï,ٌù£?'¹ÛrEÜr?šdÎ]\Ñ?'¹ÛrEÜr?îٝØ٘?±«ÈîŒ^I?¢f/"*4€?±«ÈîŒ^I?é·e°º?ÊsƒBÈ°?É"k¥?•?ÊsƒBÈ°?è(tË%z/?·L#ŽuZ<?Ï^,ÓjB?·L#ŽuZ<?ç1®K,y0?ºß
0Ð?ќ£i§
 ?ºß
0ÐAGN4FGL J1737.2-2421¿ï¨pŒ°@
F:À9Ê/¿á+ÿÀ;|ùOâ–@ |}Šsï@èËùh6J?ÀËCòž¿¢Üü@q¤?æüC͇Þ@®r/QŠ?ïË:%•»¿¿ã¾>ê¡t¿ésòí†+¿çqÿÅG¿èVþ"p?Ôåè&Åf§UNASNone?îFh×QWƒ?Èh`á,Ô?«™rˆVÒÕ?Èh`á,Ô?ïZ¶?äê?¡ã»M^Ý¥?"§©=*ÌÀ?¡ã»M^Ý¥?îJŸIm—? f˜ ¬O­?«VjæT"? f˜ ¬O­?#xn?q¿Œ´ºŒ?‰Ø·=tŒ?q¿Œ´ºŒ?íS,¯~?¸ANÚd­,?µfŸ'R?¸ANÚd­,?è¯jç)šX?Ìê)¸úÌ©?ÍBTcY–Ÿ?Ìê)¸úÌ©?ìêϜŠå¢?¨ùöÈ(?¸©ƒ¨Òó?¨ùöÈ(?ìv\=B«¡?ªGvö§GÊ?¼Mê¢÷?ªGvö§GÊAGN4FGL J1737.3-5300?æNQû±wîÀ&`'ÏR¹
À:–n6>€nÀ<)RáP@Š¿â@inù²Þå?íÐȯܧ¿‹‡¨3
ñ?É–¾ÈÓ@œÄq^'?ä «†+(¿Ú§a£‰¤¿ä€ƒSld¿ã#ý5Je¿æ"!Í°!›¿ØûsT‹sUNASNone?ïúý*&‰?hgNlhQ?FÕJ¾Æ?hgNlhQ?ïï±cdÔ@?h
ê·ãîg?`NœÈ†—¸?h
ê·ãîg?ïï0üïv½?bx'ûçØo?`Ï,"—?bx'ûçØo?ïøæÇ°êT?1é'é|?Ldàäíkå?1é'é|?ïòΐé"%?U{tQ?ZbÝð^•î?U{tQ?ïÁhÙÄh6?¿êa]ƒ?K"(Ê¥.?¿êa]ƒ?ïÕAàl‰8?zë×îUÀ÷?u_»üôG?zë×îUÀ÷?ïÙ_R~… ?aô@QOc ?sPV pÜ`?aô@QOc AGN4FGL J1737.3-3332¿ïãÁl,µ¿íã¨TáÚÀ8àòFÀ:vIë	Ï@¯'º@K•"d~?Åúq¶%Á[?Ú7ÖÛïTŒ@—›ý÷è@¨0‰à"ÿ?îØn¡Hdž¿Ù¾(Õ!°¿á¨ª®"Ó¿ës³‹³'	¿éFõŸ<q¿ïô™=SHUNASNone?ց§N.È?Ðs¾Mòì?ä¿,}Xèœ?Ðs¾Mòì?à[©ò,WÍ?Í×.7ÿSe?ßH¬§Pf?Í×.7ÿSe?ི%Š0Ï?´K%¡²ê9?ބ›´ëžc?´K%¡²ê9?ãÝá›w%?±ÁlHŸùR?ØD<É´ç?±ÁlHŸùR?»ÃÓ²w¿ˆ?½¹Ø"Õ_m?쇅‰±?½¹Ø"Õ_m?²4Jö£~Ø?¾älëT'?í¹v¡G
?¾älëT'?Ä8ÞtPE#?°›a›«‹—?êñÈbëî·?°›a›«‹—?¬F6ì·_?œ}XdRâf?î;œïÑà?œ}XdRâf
MIXED4FGL J1737.6-2350¿ï	^½>~@ÃNü½UaÀ9³ç't1*À;S~3Æ@m]–^%Ð@N€F}?ƾ—jjW?ÐÉD'@	ž³íQ@Ku&r°w¿æÞKòK?ïäÍ_ê2¿æ;À½Iø¿ä­Çüƒt¿ê2QáÊ	ú¿è
GŸUNASNone?í]4	X)ž?·«|`.Ü?µ_¶ö?·«|`.Ü?æÊ
Q,¸?ËÌÇ OÊ?Òkå]ߦ'?ËÌÇ OÊ?펢Êg9B?¡BÖ5ΐi?³Šé­¢ò?¡BÖ5ΐi?ì'ß]Éó?š‰`mQ\×?»é·¸i?š‰`mQ\×?Úÿ#v§§#?˔>{eÑì?â€nD¬,n?˔>{eÑì?ǁ¦ˆÀXu?Í~FÒò?ê–]Ïéã?Í~FÒò?Ý©Ž»^?¼ý÷ã¸þ?á+xò¸¢Q?¼ý÷ã¸þ?׳¦Ó
uò?¼qÐÁ'˹?ä&,–zÅ?¼qÐÁ'˹MIXED4FGL J1738.1-2453¿êÅu™Îâk@U.€F}À9&ÏEM+À;"£Ð_@)Ö=8ñ@.v»H@?Äx"%çEI?昚ËÈÀÏ@4‰¾ZCB@(ç-÷	?ïñýwŠ%?㲟YÌúð¿äpYߚYÞ¿ìÊXÿ°J¿ìb2Yï_Ÿ¿ê"tÔ¾2ÖUNASNone?ºcάt?Ş!ŸM?ì¿ó†'ªr?Ş!ŸM?¶êÖXš?º/µvz?í"¼å<ôí?º/µvz?×ïfÂN;?´v¿c:‰?äLžØât?´v¿c:‰?¬Ê\‰\¤`?'¦Öv¢QW?î3Z7%}Š?'¦Öv¢QW?ĒÁݟFÆ?ÎwOå
f?êÛOˆ˜.N?ÎwOå
f?'Nó.º?™'¯Ý@C?ï¶Ç›ú5Õ?™'¯Ý@C?±½<ö
_z?£Ð	ÚS°ó?íÈXaÁ?£Ð	ÚS°ó?Zd'¥…?K†ºÎ®]?ïò·Í·-~?K†ºÎ®]PSR4FGL J1738.8-3241¿à)֘}Î¿ç–Äg£}HÀ8ð"¿?EÀ:'o¶q@µ@uU«ÿ"@ZÊA¤æ?Ƒ®éŒöô?Õí3	AÈ!@	]®f°8B?ï‡îÁ"4€¿ïŊîÛëN?ïùvÿ:Þ"¿×¸o}f],¿ébü¹úb1¿ì¿Í_ï©Ç¿Çè5žrqbUNASNone?á±*0™ê'?Õê¼ùè[@?ܝ«žÌ*Þ?Õê¼ùè[@?×ÿ¬A«µÀ?ͱâ-åŸ	?ä)ß*% ?ͱâ-åŸ	?â	wÇMÃ?´×r0 ¼?ÛíÔqdz?´×r0 ¼?ÙIJC<?´ñvJ@2N?ãu[ZÞa¹?´ñvJ@2N?Òcÿ–ê›?ҐµG¨"»?æÎz4Š²?ҐµG¨"»?ª¢æ³'E?ºá\·ø?îUє÷b;?ºá\·ø?Ñ¿T¯ä?µ¥ÉqCQH?ç U¨~
ø?µ¥ÉqCQH?"cõ®ÿmš?†ªŸf½BN?ï\àRˆ"?†ªŸf½BNMIXED4FGL J1739.1-1059¿Þe¦'¾r±@%7â–é¼À9êuWšñˆÀ;r0˜N?ÿ@s¸7ê@P¸d_ûé?ØÐ\Ä|Y?á¸é‹It¾@7褙§Ü?ý¾îUÄE?ïþèÞ{Jú¿åöŸcÝõê¿â^þ]hã¿éùøuȿ뵃Úët¿äHŒ`ÌUNASNone?ì. •){?½Ínßê?¾ŽûV´'ö?½Ínßê?ÙYpNœ›,?Ír²±åã?ãSGر²j?Ír²±åã?ê8ŠŽAZ?©ëüªð_ø?ÇÕÆú™?©ëüªð_ø?Ýr¦Ž}9o?²Q™§?áF¬¸ÁcH?²Q™§?Û!$9½ˆY?ÌÍbo?âomã!;Ô?ÌÍbo?ªÌ›Mɘ'?½þR€ÖT5?îS6K¨?½þR€ÖT5?Û¨[ý?¹½IJæ¶?âq+ñöR?¹½IJæ¶?£;•jPyí?ŸR½Ïõ?îÌF©vuA?ŸR½ÏõMIXED4FGL J1739.2-2717?éPx`;K@n½ÚÁ'À9UçòÛÀ:¿Véá@Y×p"½'@¶Iû̔™?ɟSÂÊÀX?×%àº?@Õ"~°	?öãXAµ'?ïGˆÒy¿å¥ƒb¯É¿á¡—)|Ñ¿è[@*<•¿é\žÊù¿ïÿÕ"[ʁUNASNone2FGL J1739.6-2726?ѳSñÍ?ÎZiØá®?ç&|òÖ?ÎZiØá®?ÁQ™M¡üó?ÁÒòföjf?뫙¬—€Ã?ÁÒòföjf?âÛș†Ÿ?´õ}/¨%?ÚHnÌÄòÁ?´õ}/¨%?Èj';-RŸ?ª­ÐLýíS?éåv14«X?ª­ÐLýíS?Á>¬ý¾K?ÃL³ì£y?ë¾pTÀm?ÃL³ì£y?Œ-²7A­?£µ'¿!øÕ?ïI7g±{?£µ'¿!øÕ?ͤ^WöS?±ùdˆÕL?è–èj?Âk?±ùdˆÕL?yÕ»'œi?k—d"õð?ïÌTˆÝ"Ÿ?k—d"õðMIXED4FGL J1739.3-2531¿á÷'ë#ÇR@ÖûÅÜmÀ9ÚÖzËxÀ:ÉŇ^.@`æzGð@R):‹í	?ÀÄq‰…$m?ֈ$;ɄÄ@©(¿;ê'@‡rÑÙ¦û?ï÷º· "¿Þ}nàÞQ¯¿ã ³iNx3¿æ:½ …«¿íÍӒ¹«ˆ¿å¾Anµ?UNASNone?ÅH
L46?Æ1Êéòo?ê­à=lòò?Æ1Êéòo?ƒ@aˆ†?Ã.ýñV?ê[oç»Ýß?Ã.ýñV?×.›Kæ«?³4xÏë´?äh²}Z«?³4xÏë´?×Ûh[‰¹?¯nu(¡ú?äKÒ;v¤?¯nu(¡ú?£0¼P÷À÷?´[¯l±Ý?îÌô;Ð?´[¯l±Ý?Ž¥¢§ºb ?£—â. ?ï…iuSX?£—â. ?±~5=üS?¡»
Wž?íÐ9X2¾f?¡»
Wž?—ÅÄòm-F?'vˆ±²ì?ïAÑØ5œÖ?'vˆ±²ìPSR4FGL J1739.5-2929?è²À=¦	?ëÌ¢q¯À9{'±HÀ;MøԒ"ì@5#ä`½/@$Þ˜¯?Ғ(ÁÀ)P?ïûB+ºü@úô­¼fM@«À›<8¿ïÿù³>†?ïÿ~'Ø	?´ÊÅ㤀¿ì51ÛD^Õ¿é8›‡°c
¿ïÿ+#š8üUNASNone?ÙkÞh‰3ù?ÒIVY­Ô?ãJË»f?ÒIVY­Ô?ùôV?Ç"µŽºü?èPQ'ë?Ç"µŽºü?áE6à‰9œ?²™¾Í°¢u?Ýu'>íŒÇ?²™¾Í°¢u?ÂY‰7~Ø?ªâi¶åËE?ëi²àJ?ªâi¶åËE?¹×²ˆAÇ9?Çõ£êš+ÿ?ìÅ	®÷Ç?Çõ£êš+ÿ?—nGÝïqÙ?£1÷†Ð7g?ïDÁBá?£1÷†Ð7g?Å´ƒy`'æ?±–ÑÉ»ê4?ê'ß!§ßF?±–ÑÉ»ê4?{)ô¶ÕM?q[Éȕ?ïÉ­ÎYê­?q[Éȕ	MIXED4FGL J1739.7-2836?»Eõÿ1_/?ôW½;_QŸÀ9Ë
F9 À;ºB¿˜0ä@ W·¡íP@i¾N"È?Òë=%Op?ïü ¨Â@(¸®1×?ý%@œ'hz¿ï÷&b?eF?ïölmçd(¿×Xï»^h¿Ø•o¾Sã,¿ïâa9Ö»?âN¦±\UNASNone?à@>aÃ(?Ѩm%·
?߃<yDZ?Ѩm%·
?Ֆ|I¸Áä?ÍܶyÏ$?å4ÁÛ#Ÿ?ÍܶyÏ$?â-€û¬Íî?²¤‰³Æ·!?Û¤þ¦d%?²¤‰³Æ·!?Î;àၺ«?´¸t†Qͯ?èqǟ'U?´¸t†Qͯ?ÐÔòu¨Î–?Ь•Âõ?畆Å+˜µ?Ь•Âõ?ž–E"CJV?ªÉœ{î•?ïMӔßm?ªÉœ{î•?ÎçŒx–6/?²¿¸ºD?èFáÚrt?²¿¸ºD?‰}"È'õ?Û0äíì?ïš	°Ð9`?Û0äíì	MIXED4FGL J1740.1-1928?Û-'«äu@Œ¢:RÀ9E,Ñb¨À;ÀJÞJ¤@×ï½èƒb@#é Àiè?Ê©œ)&??ϲ?WÙ±@§~"ƒÖ@Árážëé?ïD8>4ï¿ãu]ÐÖ¿êøÛH"¿åŒ){D¿ïÿ>¤€}i¿ˆ5ø=œòUNASNone?ëhcTŸOÍ?Å<Uë2Ø3?Â^r­'ÀË?Å<Uë2Ø3?å8PäË`?ËK¤‰?Տ_ü6i@?ËK¤‰?ëç´¸6›?«,
–iÙû?Ãüa-%"?«,
–iÙû?èݕ×d¢¹?§7yûÙ%?̉¨¢mu?§7yûÙ%?ÞT\‰Ôç?ρԏc?à÷UÑ»?ρԏc?¶î (¡VI?ÂÝE-»q?í"+úëÕ7?ÂÝE-»q?܁(B®??¹eÕ;Äê?á¿kÞ¨õá?¹eÕ;Äê?Áöm‰_(ž?¦â¾ßJê?ë'd¨5Ø?¦â¾ßJêMIXED4FGL J1740.4-2850?ÌËÊ
ƒD?ð
Ð"¢§À9†ñ·û"À:s¯þ_ìÐ@"ù‰@? §??Չüm¤HI?ØÈáè@
'h	ԕ@{……e…¿ïÿ2Döª?ïùÍKw͗¿ÚCC ¼
7¿â˜ÜP'`¿èÔ6¸ù±1¿ïûgêÊä•UNASNone?ꔣCw­?Ë2imƛÊ?Å­s¾ò!N?Ë2imƛÊ?í³{o.ƒm?µ™;¡÷B?²d$†ñ?µ™;¡÷B?ä'ÉÖD½?´ ~Ê$?¿?ÖÚlSv…Ô?´ ~Ê$?¿?ïGÝ[²¦?ŒeÊQuÓ?ŸwWùGF?ŒeÊQuÓ?è<ôÒqɾ?Ê+rv·cÑ?Ï,¶8Ù?Ê+rv·cÑ?äèþPþJH?з}ìP1?Ö.^ko?з}ìP1?âµnùÕ:ý?¶ºFêùrB?ڕ"UŠ?¶ºFêùrB?åìpð>R1?ÀŸ¿Ð?Ô'ƒ[?ÀŸ¿ÐAGN4FGL J1740.6-3430¿îy3òàÀ5ĊÞìÀ9ùóEÀ:Í£ùZÊ@‰éOdl;@‰â¢!'˜?ÅÐ2²Ú³??Éédµy@ÿEÅÜï?ÿEù ½º¶?­ÇN¿èpöa7¿çBYì°¿äö¦_¥¬ø¿êõñ‰D·À¿ãĸ;SéUNASNone?î‹q ºÆÌ?°Oeæì?§Híò›ÅA?°Oeæì?ìIèNæöw?º…2*/å‡?½°½ˆÈLF?º…2*/å‡?ëdPxµÁ?­`€ì"U?Âoâ¾(ý?­`€ì"U?쇕ù¯Œ~?œˆýLîÜq?»ÃP2ƒœ?œˆýLîÜq?åJ 4cÀ?ÉϏ{Û?Õk¿—Á8€?ÉϏ{Û?۰҇ï ?ÒDSÜ?â'–¼s0?ÒDSÜ?àq™i_í?¸ßÁ8ƒf?ßÍ-ù@&?¸ßÁ8ƒf?ÔÔ@UýÚÙ?¶…f†Y¼X?å•ßÕ"?¶…f†Y¼XMIXED4FGL J1740.7-6750?²|>NÀ2¯Ë':)ÇÀ:ƒž…'À<&c{Ð[@ÑA}£ÄÁ@°ÚB×%?ÂVûºKü?Ï¡Îò@úœ@"0{ÈÎ;@Všó
ú?ïý«&‰×…¿äØڌ¨ðO¿ì{¯¾Ÿ ¿åЭÍ-DÝ¿îDý[5¿ïÿߞ¶ŽóUNASNone3FGL J1740.8-6755?ïH{<óa?™
‡v-8/?–ð˜hsO?™
‡v-8/?îÄ3,–ûž?©z-J;?£¼Í3 ª?©z-J;?î7ÇQÒt?› €Ñg4n?¬†óvµ?› €Ñg4n?îm‹Ê+»M?Ž«¬QÕj?©'C\hd,?Ž«¬QÕj?ìŠq¾¼ÇO?¼=·Èô?»¬r
Ŋ?¼=·Èô?ç­
âÝ}?ͯÎàßd?Ð¥ê:E÷?ͯÎàßd?çïÿZâû?´ÈÌAt…?Ð óJ:?´ÈÌAt…?âÊCÝ6I?¹8²?ï€?ÚkyòE"n?¹8²?ï€AGN4FGL J1740.7-2640?Ë:Ý
Y&Y@ÕinX£/À9¨‰ò\©NÀ;L'݃Ô@ð¿Îâ{¶@;½Ep?Ñú"å$²g?å7]ú14@‰0«½?þûþ0Gœ?ï«íßl¿⎧Þ*î¿Ø ­ŸŠõ<¿æŠw½¦¿¿ïÑdBSb¿ïäó¿ÕÃkUNASNone3FGL J1740.5-2642?ÍÈkx7ãá?ÈÿA<	P?èå!ò?ÈÿA<	P?ºî!h&ý<?¾(QdÃñS?ì¢;Òû X?¾(QdÃñS?Õ:Q¨œÊY?²f¤²ºB?åb×+±šÓ?²f¤²ºB?¾¸P`bÝ? ;C¹BuS?ì(õóó¾d? ;C¹BuS?Â~µÙ|nÍ?Çÿ¥Fú:?ë`R‰ äM?Çÿ¥Fú:?"ºÄD©?˜ðÁæÃ,¶?ﯥ	Õ?˜ðÁæÃ,¶?»Ø"ôÕ2?¥ñª8–8?ìŽDû¡eZ?¥ñª8–8?{ßÚHÈà?iúéeíÄ6?ïÈ@K¨'¯?iúéeíÄ6PSR4FGL J1740.8-1832¿ÛôW;ŒYP@kÓ^·E|À9ÌY…­S‹À;G¼PíX@´\®T@ƒ¦Mà?ÌûWϟ»?Ìs¾ÿÖ¤@öU&£ø@Dz"ø?í]ì_9K{¿Ó¥Üû(¿ã²°â
¡š¿éòÂ?U*¿ìÏ÷>^‡¿ïØÎÎ.̜UNASNone?@®W'?')YÞXd?P/Æ«ÆN?')YÞXd?ížÔeÊF?µl¨p¡?³	\ÚoN?µl¨p¡?ੁ?›Íìq'Á'?®WÆ.…Ëó?›Íìq'Á'?íÄäã½?'"ã¾e?±ØÛxâ?'"ã¾e?ë"8€Ç]?½­"ß[ÖÒ?ÃíïüâŒ?½­"ß[ÖÒ?àn͟thÌ?Ò¹ùïM]ß?ß"dÁ.g?Ò¹ùïM]ß?åS†AøóÇ?¶x?¸y?ÕXó|r?¶x?¸y?ᕰœH(@?¶ïäˆt©?ÜԞÇo¯?¶ïäˆt©AGN4FGL J1741.1-3328¿éšp²Ö½£¿ù]ÄuqÀ9ÞL¸ÒDÀ;;3$º¼@§T ¾'v@$ÖÿU¶?ъ'¥aMù?âjd!èˆ@.;|­Ñ@ÍLVšÁb?Ü3ÿ`óµÅ¿Ì-ü}¦ü¿âԃ ±¿àIÓpóˆ¿ïÿý¡UûŠ?ïV⚔k\UNASNone?éÕgG"El?Åú'îîpó?ȪbáîêP?Åú'îîpó?곕ø¿×?Â͏¤gÔ?Å1¨à¤?Â͏¤gÔ?æôOu^%û?±.-(Æâ?ÒaC´
?±.-(Æâ?í.¼¸Ïâ"? ~›H?¶Š:ÊÉk? ~›H?à?ã6?ÏõÿHþ*?߁éö9"Ü?ÏõÿHþ*?Ë970eDö?Êþ÷†"³"?é1²3æ®Ã?Êþ÷†"³"?Çó|RС2?³x˜Ç<Y?ê ëK×´?³x˜Ç<Y?Ôå쿗–?»0åûòÕ?å÷
	 45?»0åûòÕMIXED4FGL J1741.3-3357¿îÿ–ú­Ü¿ýÔlƒ¶ÙFÀ9Ä«^½ûyÀ:Ñ¢¡€è@ ¼Ü¥1þ@ø¼þ#@B–³5L?ãõ@‰]@ƒm¨z-@ã·­Uä
?ãÔ<ÞÓj¿îÿð:»?íD8>4ï¿ç.þúG¿ïóZ _†x?ïIÃ}˜²UNASNone?éèttµÎG?Ï@|z'…´?È^.-(Æâ?Ï@|z'…´?èÐp;Z?Ӓ¡Ã3Ç?Ïø¿'?˜?Ӓ¡Ã3Ç?ç).°þ¡A?±¾õO3*5?Ñ­¢ž½}?±¾õO3*5?çO}ô¢~Æ?ÉkÆh•ÑÊ?Ña»u?ÉkÆh•ÑÊ?å	õîjgŽ?ÒÜqk¹H?Õì#+0ä?ÒÜqk¹H?ÝÿK0O??Ø|L³4?áZg÷Øa?Ø|L³4?ãtߋrX?¶&þ°?e€?Ù@éÕP?¶&þ°?e€?ŶbA?Í¡'%J×?ê¾ORgoÀ?Í¡'%J×MIXED4FGL J1741.5-2344¿æ8?tè'Ú@òÒ»#WÀ9Ê:̄¨qÀ;´w K@3Æ̈́W¾@NˆÄ_@?ÑcáPè?Ý°Dä6@
Ž6A?û.'Å?ß?ÆßÅDd«?áÜlýÚ5ì¿ß±ÔÄ(¿ê[Ы~žl¿ï$ìH"É?ҟ.Äcœ²UNASNone?àTEiÁ­?Ð@á®Ó‰ø?ßWu,|à¦?Ð@á®Ó‰ø?Ëå|­5éØ?Å%	½?é Ô²…Š?Å%	½?åU)€éÍ?°á½öãO/?ÕU¬þ-öf?°á½öãO/?ÜÒÖÞë՞?°çù¸ûû?ᖔŠ1?°çù¸ûû?Äe~R
?Åó¥X@?êæ kx|œ?Åó¥X@?.ˆ_ ?£`<Pq?Eûc?£`<Pq?Ä?yä-ͪ?¯WYOžñ?êð!†ôŒ–?¯WYOžñ?œxÎøêð¡?†M}›¾
]?ï9ˆ+›?†M}›¾
]	MIXED4FGL J1741.6-3917e?Û`6Oâ[ÀÞÉâ6Á]À6ücÔÀ:cã6îª@~ÇäیX@cyú—á3?˜2™sW;?‹Ë<Sî>·?òV¦4²4@ySÙFí?í¬œuìì'¿Ò¾ku™à¿áÁŸÂ¨†œ¿âCn9œ¿ä;˽Ù¿ÐiÕOçŸUNASNone3FGL J1748.5-3912?遹vŒVï?ÌwN%Qô?Éù%ΤF?ÌwN%Qô?ï{Ž)V™?©$æ"âh?œ®:Õ,Ü?©$æ"âh?çu›½W±9?³ØõéÀgS?ÑȅPŽ?³ØõéÀgS?íºK§?¦ãí­®T?²-¢Áq¶?¦ãí­®T?çYçG×õ?ÌpžÔþä?ÑL0ýpP?ÌpžÔþä?î]z<~ƒ?·¯O"Ò]?ª.ˆ]ïåÐ?·¯O"Ò]?é²ð3Èô?·\fg¥ò?É4?0Ü/°?·\fg¥ò?é_CHtx?Àðá?ʂòßÂ.?ÀðáAGN4FGL J1741.6-2730?çIŠL
Žx?÷âCV–åŠÀ9"uÝÒ®ŽÀ:ys›Ùú@ìØwÐÇ@Z5Ö|?Ë[›\<kì?ÚÓPtŒ™×@zÄÂ<P?éB‹êÂk¿ïÿÙÐs?ïÿÅè¬ý$¿æþýÝ;¿ëTGÛ`ä¿ìŽyP¨9¿ïÿgßbP­UNASNone?ÊÐFGÅ?ÑÈ(ú0nn?éKîn:μ?ÑÈ(ú0nn?¸ó–—ßïº?¾$"Œ~ö?ìá,è…)?¾$"Œ~ö?Þ;aw`¬?´Z¬àþoù?àñbODOª?´Z¬àþoù?ª"`j2­?"µó­¼ZG?î]ÙùA[%?"µó­¼ZG?àY.ýÄfw?Õ~Í£¿ëÆ?ßM¢w3?Õ~Í£¿ëÆ?"Úy«	%?™R?›~ÿ˜?ﬖ˜"›?™R?›~ÿ˜?ƁJ˜T ?¬ï9¬p¢/?ê_­Yê×û?¬ï9¬p¢/?KÀDþ€Õ?Acúä>Æ?ïù>Ïë݁?Acúä>ÆMIXED4FGL J1742.0-3020?îòÞúvÔ¿±ƒÙÓ-©À8de+ÓÃÀ9 çJ&"¿@¤_ݶ)@ùGÏ¢j#?åãM"M2?Ò'5ø	'@ĸF-
û?þ FnÏ@š?éñUbˆ
{¿ÕAuÁ"I¬¿è±ÿ÷œ"0¿çù΍—,Ø¿ê«-u"›¿Ò¸`Jã(UNASNone?ââü‡Ù?ÔªŒö?Ú;þðMõ?ÔªŒö?ã4˜XÚjM?ϵì$oº½?ٖÏNK+f?ϵì$oº½?à#«}
±y?·
¶ÐJÖt?߸©ê?·
¶ÐJÖt?çmÝÎRô?´°–£Â}Ä?Ñ$DcÃZ?´°–£Â}Ä?å<çû¸ƒÑ?ÓñÌlε?Ն0Žø^?ÓñÌlε?º"$ñ1½?Ãɦ3¨E{?쭛aÎYÈ?Ãɦ3¨E{?Ò4ay 2™?µ|µŒO?æåÏC/æ´?µ|µŒO?°e;Õ)y?¦z3Ji^?íÿóX…ZÑ?¦z3Ji^MIXED4FGL J1742.5-2833¿Ð!¢ä¾Rƒ?èÃoõPÀ8Â.jÑÀ:"P\8æ@i.r.E¹@(¤~Ïé¸?É@h:{üÑ?Õã*Ý#\&@qìb"IÏ?údDÊ=Ñ?é"L["e†¿Üaq¦3[¿ãONâ'/=¿èÄ1Bm7ç¿ï;_A"Û?ÑÂìúUNASNone?åsu^Y?ӟ;	}k?ÕBåáN?ӟ;	}k?׌??QŒ?Ï_Ž	\có?ä9à`t×:?Ï_Ž	\có?Þ¿o.êÇ?¶òåÓ=†?à HhŠ¿?¶òåÓ=†?Ú®|}ì¯?¸˜Ú©Ýž&?â¨ÁûÁ	©?¸˜Ú©Ýž&?åWZ:;î?ÔÉ?3ǂ¶?ÕQK‹ˆx¤?ÔÉ?3ǂ¶?¢ŒÝ †?²$]-ÊÁï?î×>1áEø?²$]-ÊÁï?ğyYªª?¯/Ÿ¾—lþ?êØ!©•\•?¯/Ÿ¾—lþ?ˆ¤ú2Òx?~_îiâí*?ïl]ó.?~_îiâí*MIXED4FGL J1742.8-2246?ÌÔv?Þx'@
ñqýs]ÆÀ9°(¼·«ÓÀ;"bGóµ@Š•{&çË@;'÷
è÷?Ðl8¢Þ¼¹?ÛþÍzò@Ã#·;k@G91úÎé?ì«ÊÅ㤿á˜Tà'^¿â[óEÝYã¿ê*€Â2?¿îfd¸ç<»¿ï¸àâ"UNASNone?Îð€V㢸?Í
s8(\ã?èCßêGR?Í
s8(\ã?×9E å­?ÊC77NËÀ?äc]u¯)?ÊC77NËÀ?äF"qh"?´Nhšëu§?×r÷Ù.Û?´Nhšëu§?äáw´lƒ·?°;8ʨ®€?Ö=—&ø'?°;8ʨ®€?±#ëHŒ,?µŸ¡¿¦—?íß{'¤¬ê?µŸ¡¿¦—?Ÿ$h…ž'°?±'
:?ïÜ»àÉâ?±'
:?ÃA"®Ô?¯ûd¤cÿ?ë/œ:TK?¯ûd¤cÿ?¹	|½/‰?¢<ã.¨?ìÞÐhkVï?¢<ã.¨MIXED4FGL J1743.0-3201?ßfÈäi.¿òlÛzåylÀ8òñÝ'ŽÀ:i›€#¦Î@;MÄ®ñ@e|áÒîO?ÎÔ6SÏ
?Ñ!Œ!‹ëÜ@2€l'Ð@¤æ'™ð׿ïèùôMDV?ï,™†Nc:¿å!"dƒã¿æ1Iï7Zà¿ç~Ê-ëÌ¿ïÿþøþ"UNASNone?ëë¦4e@?ÆØ4¡"²!?ÂQg.k?ÆØ4¡"²!?éºËXiµ?ÅÖý ìMŠ?É"ÒžY-?ÅÖý ìMŠ?ä	¡7ª´?·ñ?¶Jë'?×ì½ÿª™?·ñ?¶Jë'?뿂Ü`5?¦·ðÃ]H—?ÁôŽ+§?¦·ðÃ]H—?펓IQ
g?¼¨g)3?³‹e³¿ÞÈ?¼¨g)3?ÙîÒèèÖ?Ón
W_?ã–‹‹þ•?Ón
W_?ào´ó‰œn?¶Ž‹êÈV?ß –ìÇ$?¶Ž‹êÈV?ιM¶c¡2?¼Þum±è?èQ¬'g´?¼Þum±èMIXED4FGL J1743.1-3049c?ïùÃy֟x¿á"<5:tpÀ8®XŸÔF>À9ô"Ÿ^Õx@—'Ýè¨ö@@Ëò¤Î?ÊÈË5rþz?Лüà»Â@éý_;Ð@Ðyí¬Á?¿ïÒü›K ?ï½pŸM8¿çh*á«I¿ã'™îLÏ¿èõ¿¿óö\¿ïü\§ ÃZUNASNone?껫IÅEð?Êٖx–®r?ÅRØêèA?Êٖx–®r?åzž;ê¼Í?̒=š?[à?Õ
È*†f?̒=š?[à?ßvmô¾ó	?¶Â{q,Ái?àDÉ †{?¶Â{q,Ái?ëFu^œ²?«èDÏEL?Âæ+҅7?«èDÏEL?á쪹¸¯?ÑRNY²×a?Ü&ªŒŽ¡Ì?ÑRNY²×a?É:©öÓ?Ëo&òeÁ.?é±U›úK?Ëo&òeÁ.?ÒüöòKr«?µ×rE>cî?恄†ÚFª?µ×rE>cî?Ŕ¹]â¼×?¸Óº6âC?êšÑ¨‡PÊ?¸Óº6âC1MIXED4FGL J1743.4-3123?ì_&óû:¿ëú¾ï>'À8â֕£jÔÀ:@±NÂó@ 4^lFû@Ú½]Äu?ñ)ŸÖÊ|?ÎÕ< ˜@D¿ÒéF€@ßÿtißB¿×ù\B 6?ãsʒ`¿æ^B.ù"¿å#•0~M
¿ä{õO¡S¿ìä"CÆÿ-UNASNone?éÌ*Í!ö?Έ³
Œ~‡?ÈÏTËx'É?Έ³
Œ~‡?íj}'P¯y?»ÖTœÁø?´¬Å¼?»ÖTœÁø?ãP<7,«É?·Ðxœiš³?Ù_‡'¦¨m?·Ðxœiš³?î 0V?•.(Ž<äÐ?¥þèÀ¯˜?•.(Ž<äÐ?èŽÒ1ÕSô?ËØm¹?ÍÄ·8ª°1?ËØm¹?哷‡!?ÒñPš¢-?ÔؑÂñ½Ù?ÒñPš¢-?âÜ`®kÃ?¶p»å—öŒ?ÚG>£(ä{?¶p»å—öŒ?àÅþ¸	ú³?ÅÓhN=ƒ?Þtì
™?ÅÓhN=ƒAGN4FGL J1743.4-3406¿î_pö.½ÀlZßI§À:ZKÄ#°ßÀ;®
9>åï@áÑcµ\@Â=&Ñü?Øéq}ñg?ãÜ|m8è@y‡Æ2~Ø?óï•!îZ¿è$EÅ.î?ãü`£®ÆR¿Ï|èˆêö¿åÍ´Þïd&¿êŸÐJ/Îû¿å¾§°³'UNASNone?æd ~Ç?ÌOž+œ?Óû7¿ñr?ÌOž+œ?×k>šÖ—?ί¢  0?äJp`²"µ?ί¢  0?ç¤åm‹&m?±fÎìç¾M?ж5$é³&?±fÎìç¾M?×b'ûìÔ?²އz×8?äN·q'	–?²އz×8?Ðæ_¦¿Ù?Ì|€lÞ?çŒÐ, ~?Ì|€lÞ?¯U½<ñ?»'
Ô°|?î
¯õ>A?»'
Ô°|?ÎÉÁ¬ªØ?µ5µ›7;q?èM"Õ\
?µ5µ›7;q?'|0²bXß?€‰Oó¨ñ¶?ïlzz«©?€‰Oó¨ñ¶MIXED4FGL J1743.4-2406¿çÛyoÏé@yߖÓìÀ9¢"'¡WÔÀ:èñ«©f–@ê£q^¼ú@Aë¾íç?Ê{‰¹&Ò¨?Ïe7ýO1@EÇ
âA?ÿNç àö%?íQŸ?ûs¿çzä7Lh¿èZ<ŒxHç¿à"à4ˆÉ¿ïÿþøþ"?ã8}àU•´UNASNone?é"öÎí¨(?È®À-"GV?Ët$ÄI_^?È®À-"GV?âÌã Žý?Ðr²‹>H?Úf9Ó¾â?Ðr²‹>H?é^`O˜f
?°'[£
?ʆ~Ážg×?°'[£
?ë%€-?†Ü?§ÀÞÝêƒ ?ÃiÿKä?§ÀÞÝêƒ ?â#9«ûÏw?Ïæ9¶Á-î?Û¹Œ¨a?Ïæ9¶Á-î?§mÀ2@·.?¹6ðw¹Ú^?î‰#üÎ6?¹6ðw¹Ú^?Ùݲ¢"?¹SÁ¦±µ?ã&®óüo?¹SÁ¦±µ?È}¨ˆ†?´yø«?6á?éý •ÝÞ~?´yø«?6áMIXED4FGL J1743.6-3341¿èåxÑ^=ÀÝ!ê6À9•$Š#À;‰¾ZCB@ m™Y_@õ~íEé?è&ûíKÈU?È/«©¼|s@øZðŸ@[2\sž]?ÁHç$'Ú³?ènæ4'¿Ëñ.Uþº0¿ä5çéóN¿ævñ~\ý1¿éIO4¹ÀUNASNone?ïð-áü?µY¥$¦?¡ú>´–?µY¥$¦?ïtÓo0íç?™2°ûa¿ö?'e'Qß?™2°ûa¿ö?îcDƒ›3*?Ÿ=}VEp?©Ë·Ã¹^?Ÿ=}VEp?ïR©‰aú,?€¯ 'eS‡?•ªÎÕxˆv?€¯ 'eS‡?ìªçï+á?À­°$Óýv?º¨À† ÷?À­°$Óýv?í3ø Bo?Ài£¶í¬/?¶`;ôµº†?Ài£¶í¬/?ê1­æÇd?°üÔ{'©ƒ?Nj9Hdâr?°üÔ{'©ƒ?êê=a@?²7
~àß?ÄW
{·?²7
~àßAGN4FGL J1743.7-4321¿Ó2? ÝcQÀª#žj¹²À9ËÍiª¾…À;òHv'VÕ@äÖÈN7ñ@^½$¹?Á–I˜z_Ã?ádv6¾/@9ßÞè@Ž÷Õ:?豈bîпšàRe¨{_¿ÞƧCÑ;¿éûß¿˜±½¿ïցz"ð¿í¤{	‹™ýUNASNone?Ú½ÂÔã?ÈVÑàS•?ëzPJÇ?ÈVÑàS•?Ôפ#,Í5?ǬFôŸéY?å"-îi™f?ǬFôŸéY?ÑQ4¹Mǒ?²ÿ-i'T?çWe£Y7?²ÿ-i'T?Þv¼âkfù?°ù"³Ïžæ?àÄ¡ŽÊL"?°ù"³Ïžæ?¡,P}âR?µW¡¢Ëž.?îí:ø=W¾?µW¡¢Ëž.?¬)QúFù&?´¾ÚOO0?î=jà"˽?´¾ÚOO0?™ÅG½ñÍ?Ži4ùíþ?ï1Õ³'?Ži4ùíþ?¨ùµ€…?H'¤T‰?îpgµ¶?H'¤T‰PSR4FGL J1743.8-3143?è#5½¦Œ¿ò:øúRAÀ9['IWbÀ: ¼X
ƒ@!]úŒÎ…	@Õ¼{`É?É2ØÅS†»?Ÿ!N%Ê6g?ße)ÛÃP@Uvꚿí!ñÂO›I¿ž-QûRú¬?è'_³Ä¾¿å'§¢pØ°¿è<Èk.L¿À•¸#®UNASNone?ïº^+%Ü?ŸòZ;dùã?hu;î§?ŸòZ;dùã?ïÃý]ŽP?'{šXšñ"?~Q+Gõ?'{šXšñ"?ëG¿"?® Pš†°\?ÁÃöᡱ?® Pš†°\?ï˜Îœ@ú?+*œ|ö?‰ÌXïÁ£?+*œ|ö?îÒ¯>¾Ï?°¬Ô£Ÿœ?¢ÕÊÞ?°¬Ô£Ÿœ?îÑT¡Ëtç?³A?Î<²?¢êµâlʘ?³A?Î<²?ë%gFqd­?²dA÷ÈÙ5?Ãjbæ:mJ?²dA÷ÈÙ5?íޙ:E˜ˆ?¨×ú?±6/??¨×úAGN4FGL J1743.9-3539¿ã%—ԝ{¦À	¥%1À9Í:óñÔÄÀ;bʤÔ`?@1¡¸¡ó@‰ÂÁ±Ø?χ?ÏÏ?ä	pA0¡Þ@+vö×bR?ûç­ôDŠô¿ëÝâ¾ü˜?ï2«M÷¿éÂ!øù&¿é©yámm¿ïüpßFI¿è!8>µÈNUNASNone?î¾ŽyŽ?«®ÅB?¤7ØË?«®ÅB?ß©Y‹?ÏeŠ²ÃY?à+Sw:7ù?ÏeŠ²ÃY?ër•Þã?§…äŸÁÍ?Ú5«ˆ"s?§…äŸÁÍ?à'•uêà+?³"3+M! ?ÞÚÕ*?«?³"3+M! ?ènOùèc×?ÊËùo˜?ÎFÀ^p¤?ÊËùo˜?¹Û–Oskï?ÃÂ|mJ‹?ìč6''?ÃÂ|mJ‹?Ùüs$D?¸ÔtÈ4?ãüÆ~mÞ?¸ÔtÈ4?¢(Î.»n?'(Τ7?îÝsYN?'(Τ7MIXED4FGL J1744.0-2504¿ïù§—šL-@ƒá†˜5À9BÍl.ýDÀ:¨ÙRîº@¦9kÜr@§"~§¥Ì?ÌÓ÷8†.X?Í>@,•à@²Å"Ùîô?ð±BøΊ?êÑr¹[¿ç¡ŒâÑñпèÉaÔ¿èç¤T¿¿éñþë-
$¿ðUNASNone3FGL J1744.5-2506?æ-à'®'ò?Ñ7æl—>1?Ó¤>ú¢Ú?Ñ7æl—>1?Ì—¤Þ?ǹÙ*(H?èýÚÈœ?ǹÙ*(H?æR=›R<Ÿ?³à¡i<r?Ó["É[†Â?³à¡i<r?ØDàÒ	Å?³F,Ýt3?ãÿ]–û?³F,Ýt3?ÞÀo<Ð&?ф¾Zï?àŸÈ9a—í?ф¾Zï?"‡PÑ/±>?ªheOR2.?ï[Åy­|6?ªheOR2.?ٔâ$Í¿¼?·6ô¬ç^†?ã5Ží™ "?·6ô¬ç^†?'·žu#×?z<1‹Ÿ¥?ïjC;š?z<1‹Ÿ¥MIXED4FGL J1744.0-1311?æïÐ!ëã@ çqdÇ)öÀ9®ù–Ys9À;Tpš@(żãÊ@íqåöi~?À‡kŸ‹K?Ñ"ÌHBŽñ@PLýߔP@‹È>?ïÿº*2Ùq¿À¿1ÄPÉ¿àÖŸd´µ¿áê2¾™-c¿ëÃé.,c5¿ïÿŲýîUNASNone3FGL J1743.9-1310?Û/:Ï£…š?˺bñD"?âhb˜.=3?˺bñD"?×	– ÚšZ?Ç÷£"°î?ä{4¯'²Ó?Ç÷£"°î?å¿óöåؕ?²²Þ҅^Ô?Ԁ4NÖ?²²Þ҅^Ô?å\gtƒ_›?©æŠïºÞ?ÕG1ù@É?©æŠïºÞ?§¯¸éæÅ?¬3ßFB?î…qSÕ??¬3ßFB?¦çÛºß)?´ª‰eõ?DŽ?´ª‰eõ?½&M­Ä8?ªENëTà?ì[6JGy?ªENëTà?Ĉ½C?©vuÕ©œ?êøüüP¯?©vuÕ©œMIXED4FGL J1744.7-1557?ˆ>͔J@Ÿ§¨PÂÀ9ybA=·ñÀ;m§<ð@"ᷕƒ@ìC9+?½º›ÇÇ)u?ÏõðÝx@®@Îގ–0?übE1¸^×?ïÏXBaNz¿ÝqÍbHõg¿æ(Æ}}YG¿â£Å&p­¿íPA`ó`¿í±P$QïUNASNone3FGL J1744.8-1557?Ü|ñ(‡ð?Ê|Nb¨?á÷Á‡k¼?Ê|Nb¨?ÄOmæãNn?À,±¦¼Ô?êì$†G,d?À,±¦¼Ô?çLÙ½K$—?°þåt¹¸?ÑfL…i¶Ó?°þåt¹¸?ØÀдÁq?¯;:gÕ³C?ãŸô¥ŸH?¯;:gÕ³C?k7
ÍN?Ÿ íSˆœ?ï¦GÒÒu?Ÿ íSˆœ?‹ÒTDQê?—\­âC/?®Ó<¨?—\­âC/?É'*L•ì?¯8äàÛE¸?麶5lڅ?¯8äàÛE¸?œÞ0ºñ&?†c«/Ÿÿ?ï{».·?†c«/ŸÿMIXED4FGL J1744.9-3322¿ÚåN¢¿!ÀÎú¤vlÀ9x ]Øù+À;!ÖÜñ?@ES#há@Nc¥ÁÆ	?Æe
›º[0?ÝĄ^žò@ÞÔI˜Ð?þ§/ç¤>Ž?î&mó"¡ë¿äu°»õ4¿×Yӟпèi¢#¿ìpâ ôÈ¿ïôè_Op×UNASNone?Òy,ŽuÆx?Î#v^£pÕ?æÃi¸ÅÄ?Î#v^£pÕ?Õüsé†ÁÑ?Ê}ò<P›×?åÆ<Ÿ?Ê}ò<P›×?ÜXë+æ|?³´N¡ÉB?áӊjõB?³´N¡ÉB?ÙsNú—"ã?±RˆÊ'«?ãFX'´6?±RˆÊ'«?§ª!V:??±d¦ÔN?î…^­Ï|?±d¦ÔN?©§»Ívü?·gÁ¢z¨c?îe"C›°?·gÁ¢z¨c?¶ÜÏÝO?¤v¦™jh?í$fµšÆ?¤v¦™jh?—\þ§ž¸?"å%
ù€?ïE
ìJÊ?"å%
ù€PSR4FGL J1744.9-2153?î#œ´£'ž@_j^B«vÀ9•
ÿÀ;o#¤I÷@0–¤Ç @DeÀN9I?ÐҋÿH?ϒ¤g"@í¶^Ì>2@GºÔ§¸¿ënM?ùÀ ?ëÑÇ]w)'¿âü¯þàÆ)¿èêÂKiŠÞ¿æa@AŽ•¯¿æžë/ŽcUNASNone?î"#q?ª»§Ýë]P?¦Î_\¤´?ª»§Ýë]P?äã*ËÊ]?̟¾:§Š?Ö9÷ªhkF?̟¾:§Š?ì/é(ð[•?©ž×eôü?¾€¶¸}#[?©ž×eôü?ëÀ…Ò΀?£¾±¦'?üýè´Æ?£¾±¦'?ㆲMçáÈ?Ì'ÌH~°?Øò›d0<o?Ì'ÌH~°?ÁþW5"W-?ÉñÔÆ7Ô¥?ë€j2›*5?ÉñÔÆ7Ô¥?à×û˜ÖêÍ?¹â&»?ÞPÎR*g?¹â&»?ÏÄMˆ…0?·P8ç"?è9ÎìÞ´?·P8ç"MIXED4FGL J1745.3+2338¿âëaÀíÏ@8~
"¾@BÀ:T3‹GÇ?À<*»êý9|@Mheïóî@`êžnëp?»
míq¼¿·&¨
u¤È?÷¸)W^Í?üàcR4ֿ°£?4É¿åmbÙéë¿ìŠtBrq¿å™Þ"Û¿è;?Á¶ï?âÊC…ÎUNASNone2FGL J1746.0+2316?ïÜÀæ˜-'?~,ûøê¦?qŸŒÉæ·.?~,ûøê¦?ï\"OQï-?¤o·†¢?"ov1¶N?¤o·†¢?ï2'¬6ˆ?'Èc»Ï?™¯¼Šy/?'Èc»Ï?ï½t']è¾?jAÚbü?€¢ßjíŠa?jAÚbü?î¥(æ~$?©#W…
u¨?¥®u¹¿?©#W…
u¨?è»åÏ'E?Ë°ÕØ0¥‡?ÍhÃbë³?Ë°ÕØ0¥‡?î'¢iÝûZ?¡+näˆW?­…Ùd³ÿd?¡+näˆW?ë ä:ýP?²?Ù7ñ?Ã|oÌ
Á?²?Ù7ñAGN4FGL J1745.5-2249?Þ÷t¡ù §@	šxš:À9ÙéðÀ:³m—³Œ@_#·SÊ@P:ÅΫÊ?Óµ^>J?à™ØZiÙ@	z™ÄaÄ@@d"µÔ㝿ï·]d_%*?ïñ"Á"g¿ëMa²¢¿ð?ïÿû-2h2¿ïí}±«´UNASNone3FGL J1744.7-2252?êPGoø'Õ?БûÿÚ2?ƾâ@ôª?БûÿÚ2?ç kRçâ?њ™‡G?Ñ¿)Z0;÷?њ™‡G?ä‹öÔH?µç²4sn?ÖèâWoö?µç²4sn?ï©ÔU¾^±?…Ç"y…W6?…Šê"×ï³?…Ç"y…W6?ç;'µjtW?ÑÈüs-Ÿ ?щ°•+R?ÑÈüs-Ÿ ?ºÄö¶øqŽ?ÇÇR"²+â?ì§a) ñÎ?ÇÇR"²+â?Ýè'&Cò¯?¹½º.(?á¶ìÞ¨?¹½º.(?ä|ÔȪåX?Љmy ?×Vnª5Q?Љmy MIXED4FGL J1745.6-3626¿ÄŒÛŒ…TÀA&:ý,À9Y©mL3µÀ;KkÊSuÉ@}Š/™J¿@|­€k`?Ŧd׍?Òåí/Bä@…»¾‡¬?ÿ¡?¸§¦Î?ï¤Î(™Ò¿éšÌ¿¶¹»¿ã¥@@âÉ8¿ânøÁG]¿ï¡‰R#¹?ãJò|‰¾UNASNone?ï`š#y¤(?"²žÕ(?"컈4u?"²žÕ(?íµºÛøR¦?µ}2wúÍ?²R)aƒÎ?µ}2wúÍ?ë"ëSíà:?¦©r՚?Á°R°H?¦©r՚?íÐf†‹Ž®?–4 Ÿñ?±|ËÉ뼔?–4 Ÿñ?êûCù\«Z?À—"!Ƶm?ÄðR—?À—"!Ƶm?ßÀž*ÍÞñ?ѧK8b?à°ê™ˆ?ѧK8b?á-nŒ"gD?¸Ö¶N"Þ?Ý¥"æ×1w?¸Ö¶N"Þ?ߧýNR|?¼Cw'm›ÿ?à,?XÖÂ?¼Cw'm›ÿMIXED4FGL J1745.6-3145?ë`U8ÒÀ"¿÷¨Ã ¢7À9·k;¸=À:׆¾Ë'J@‹øyMô«@Qw~¼ž?Í7•˜ƒ%?ÙjÈ˶L@7Lg"t@mºB±€?çÇ_¥'(¿á£tä®k¿â(Ùþc´¿å\ƒÄE>ο煇"Ý—ö¿ïÿÓà<k@UNASNone?í^¬Á±
?¹æ=iË~L?µ
™ø¬R?¹æ=iË~L?èv	)§÷´?ÅzÉ+ÏÞò?Î'ÛY`!1?ÅzÉ+ÏÞò?é>Ùøoy?°$_°Q²s?Ë›ŒB?°$_°Q²s?ìe4¯…?¢'b–d§?¿ôÖZƒóÚ?¢'b–d§?é!˜è* ?ÈIû'å?Ëyœ_Wå€?ÈIû'å?Êq7§ÙoÀ?ʹÔ9Jù?éc²	¤?ʹÔ9Jù?áãµXUÆJ?¶_H?Ü8•OTsl?¶_H?Î
C½¼[?·æÐÆ£à<?è}}ïé?·æÐÆ£à<MIXED4FGL J1745.8-3028e?ëŽÂiá4¿êÈè§æ›À6ŒŽž"Ô^À9¡PþU0@ lÒ³k§Ä@æJ>ès? kæ­ôo~?˜ëã=|?õ×??ñ/Q|I}?ïIše]R¿à
Õç'Áæ¿â#揲¿å$;´4ç¿âÀœ<âž¿ÝŽèÑQ­UNASNone3FGL J1745.1-3011?éa^ó¼‹ó?Ò*˵?Êz"1
Ð3?Ò*˵?éHt@ÉÐ?Í_$P¨ ?ÊÞ.ÿœØ¾?Í_$P¨ ?â™â·š¶z?´åàç ?ÚÌ:Ê"?´åàç ?Þa)êÎÚ2?ÆH:5rÜ?àÏk
˜'ç?ÆH:5rÜ?êß-Ö·?ÏüŠ¦Gä?ÇðƒH§í"?ÏüŠ¦Gä?ß½nrŠ??ÕS¨ñ2÷?à!HñFºá?ÕS¨ñ2÷?æÞvb²Ò¦?»g"¯¹?ÒC:šZµ?»g"¯¹?»áÛð´¼?µï]t¿ƒ?ìƒÄéh~?µï]t¿ƒMIXED4FGL J1746.1-2541¿îŽÖOµþ]?ùMë­òíÀ91áìï'À:ö"o³í@n‰šs@1*å†×ö?г ž†~?Ñ!
Gé#@
MFðP?è
ۉº9³?ï±K(¿åV…í	¿åǐbcL¿ç§/^½O¬¿ë!¿îB¿ðUNASNone?×éc1ŽÔ€?ÓòÓM*¼R?äNg8•À?ÓòÓM*¼R?Áöàòs¥?ÂÓ]pI?똂GÃc?ÂÓ]pI?á¤BHü?µu#»Ã{p?Ü·zzÅn	?µu#»Ã{p?¹ôÝtîG?¢èpØ3?ìÁ}Qb7?¢èpØ3?ÛLh"Ðk?ÓªHñéðR?âY˵—ôJ?ÓªHñéðR?XÈF"ß­?¢'²(Z?Þójñ?¢'²(Z?Ԋ½ Vn™?¶^s_À|T?庡/Ôȳ?¶^s_À|T?c؊Ucö©?WdZ²zÿa?ïì'uåµQ?WdZ²zÿaMIXED4FGL J1746.5-2019?×ùG%û´Ž@._¢ýÆjÀ9l~|áœÀ:Ø¢xelk@µètž›@.ƒþý¡?ÒVñé¼Çœ?іé;ƒ)@	±ÕšÑ§þ@€¹xÝ?á7¢~D©}¿¿K¾ß8¿êTݧæcw¿å›ã@+¿!¿èSZ_òÙÒ¿æìa¢—oUNASNone?íáÂežH?¾"@þ¼¢Í?°ñìÔWšA?¾"@þ¼¢Í?æAæc2?ʵvѺêš?Ó}à39›á?ʵvѺêš?ëWÀ¨ž'?®Å˜Ðã‰?Ãú ý]…º?®Å˜Ðã‰?ëü̵-|n?¢x<
·?ÀÍ+JJ?¢x<
·?à›CC÷?ҡŵßÓî?ÞÉÅyyò?ҡŵßÓî?¼Dwð
?ɳ jûîÆ?ëPîþâý?ɳ jûîÆ?å‰Ñâ­¬?¶5aª¢§÷?Ôì\:¤§Ñ?¶5aª¢§÷?Í+ž`Ë\?¶%òî
ó?èµgÍ;)?¶%òî
óMIXED4FGL J1747.0-3505¿ïΝöºKÀ³~²†fÀ9;AÖNVÀ:ð~gäì@¨ç ÐH@€"Ýz™ú?Òý¤Ûìû@?àž«QR+@3¡/?ÿ¸†^©X©?î̎^''·¿ÓrP¿á¿ã@Š3Ë	¿ë©Ùîm¿èˆ"#8m¿æ)7fžšŠUNASNone3FGL J1747.0-3506?Ô³Wžm-?ÑM wÍJ?å¦Tx°Éj?ÑM wÍJ?É~Áo)68?Äh¸Ž À?é O¤5²r?Äh¸Ž À?ß­»âY¸?³á&}š?à)"pÓ$?³á&}š?Åy:^J¹?­ò"ŸžZ?ꡱhmQ½?­ò"ŸžZ?ÄKÔó?†?ËSvþÏX?êú­
Ã0?ËSvþÏX?¡ÖÉYÞ?±Ýh‡p%?îî"8¢?±Ýh‡p%?Ôd®V{H?¶ê"Bs–E?åͨÔÂ[ý?¶ê"Bs–E?cî˜æt \?_Çæ=ÌR?ïìgË°?_Çæ=ÌRPSR4FGL J1747.6+0324¿îü"J|ü@/{À6âëÀ9®Hn-ÛÀ;¶·»*ä@™Km¼›ý@Λ¤5Õ?½µnryo?Ê0¬O·x@
"­äª9$?ÿlyöf#K?È{ø^v¿â_N_¤¿à©áæ9…]¿ÞZ؍u¿í2wKø¿ïÿ⾦™\UNASNone3FGL J1747.3+0324?à1?͗ÅP?Ì6' %FX?ߝ€dÐu_?Ì6' %FX?áٝ»<V?ËÝß×t?ÜLĉ‡RÅ?ËÝß×t?étá¬ü?®ÏŠÑ±ŒJ?Ê,yOøò?®ÏŠÑ±ŒJ?é^š3aE.?¡¡ŸìQÉã?ʅ—2zëG?¡¡ŸìQÉã?°hRíSN2?²"ÄDSq?íòõ¢G×Ê?²"ÄDSq?ºßF/±–?Á\êšEĎ?ì¤W:	Í?Á\êšEĎ?ÑI‰·àgÅ?¸ú›4öB?ç[;$Ì?¸ú›4öB?ÑñlÐt?¯¥¡ßÕ?çrýI—Æ?¯¥¡ßÕMIXED4FGL J1747.7-2141?ûä¬+@
½¿cíÀ:ÅÛAÖÀ:õ‹QØ9è@ð_ŸLáÛ@èIåý{?Ô$yÜåɞ?ÀmŸ*R9?ðfÝR@ª¯³…S¿Ð€¡öµT¿èù›ÍP€K¿æöJßø"¼¿ì7ûþé¿Ê$xs'.¿ïõŸŸ1öUNASNone?ïÒ;w-? ÏM' Q?vâu5K8P? ÏM' Q?ïook«t?¢_IÌË­?'¥iɂ?¢_IÌË­?î}|h9?ž6Í#´»?¨(9ß{?ž6Í#´»?ïæ2t?[ræúFÃ?iâïá\?[ræúFÃ?}Î?«Dh{ôªþ?¤^O"Œ<?«Dh{ôªþ?éö¶Ìôÿ‹?Êè¼âžñ?È%$Ì,Õ?Êè¼âžñ?ì	¦-7?­™ù'?¿ç²Î–Gø?­™ù'?î(7¶>"º?§Éðé_ö?­|"Ÿ‡P^?§Éðé_öAGN4FGL J1747.8-0316¿ê±ü,is@)f+®´À:ÕõbLMÀ<
Ê7Ǫ@!êK¸»?ýÓ
ÔoX?ÓÞõCc'?Ó¬¹1–?ùC,Tò œ?õ`¹ÿÉ¿ïùæuë>¨?íK@š$?è6x—ÁRE?à'՟Ú%¿ç½ûm#D¿ä÷ëÿ—û4UNASNone?ª¼`?¤à$_´/B?Š—•Ðè?¤à$_´/B?ë{ãKûgP?Ɨ8\NÑ?ÂrÐb¿?Ɨ8\NÑ?îÍ}(;U?–ñ_…é?£(/þX1±?–ñ_…é?ìè4ê˜d»?¢Wû2µ?¸¾X©òÿ¨?¢Wû2µ?ï–3ô׶?'-—ñVx?Š~óÊf?'-—ñVx?äċl%?ÓØÞ0ªö?Övé'õÄ?ÓØÞ0ªö?íV«)Ü>Ò?¦þ
Ñ=¹Ž?µJ¦²gãí?¦þ
Ñ=¹Ž?挖!Å?Ã)æDíñ?ÒæÒŽÂv?Ã)æDíñAGN4FGL J1747.8-3006?ÜÈP©ï/׿ð}'@.Ä9À9ÚZgT£À;‡º.d—@ Îî™Ñ!ñ@$½Ÿ2_Ï?×}Îâћê?ïRú®‡gh@ž–›¸WË@¤öí1Ç"¿ïã%Ô¥ß"?ïgòPµû¿Ø–8ù€Š¿"Ÿ\èä0¿ë¹ýßÒ¿î女©UNASNone?îµÙ¡q?±¿|hÚ«?¤®ÒcU3?±¿|hÚ«?é	ÏÊᘿ?Ë`L_Ãλ?ËØÀÔy?Ë`L_Ãλ?èÕÐaàMf?®fþàáî?̨¾x~Êi?®fþàáî?åi&o<Ï?·á*6wp?Õ-³Í!†c?·á*6wp?åö߁¥?ϙ蜿œk?ÕÆ@ýÔµ?ϙ蜿œk?àŽ—eóS?ÓŬÎeåH?ÞâÑ5èY?ÓŬÎeåH?â

ä³ã?µ‡119?ÛÇëä6˜:?µ‡119?Æ°ßÓ²«?·×Y0²u??êSÈ{Õ?·×Y0²u?MIXED4FGL J1747.8-1827¿ïƒì"ß4@æ¢nTqqÀ:Qè·§À;Ê×)G!'@Ÿ6çrÀ@8âºtÛt?×¹vCS;ç?ï.À½të@ß«ºbg@é—M¹ò*¿ïÿ*b{ö?ïûd;¿êPëHD½¿äeÛ&+ã´¿ïÿÿÊPË?ïþá˜á¹UNASNone?Ñ'í÷·(˜?ÍûFï ?çl	$k´?ÍûFï ?Ô_"7ˆ?ËûÑ»&º²?åôÐ9=ä<?ËûÑ»&º²?äc>rpN¶?²œ›<v?×9ƒb"?²œ›<v?â´F.ý?·mþ>T'Œ?Úz—ós¢?·mþ>T'Œ?µÀUԂU?ÆpýE\øÌ?íGüÕuö?ÆpýE\øÌ?~Úβ? "Cn"?ï|	)¹%À? "Cn"?Ռíh¦?·9ÿr3ä?å9ù‰K÷-?·9ÿr3ä?«LÉåß?œ"*É÷B?îK?£¦Z??œ"*É÷BMIXED4FGL J1747.9-3224?äø]å–û¸ÀÔèÅP׉À:¾¶‰"iÀ;?"øS@+ƒ«›¤·@Ãf½Ì?ÑØýݐêI?Ûnàˆksì@	ÉrŠar@€Ì T‰D?ïðvŠ ØR¿çu5×RaÍ?˜ y
'¿ã5"÷{Í¿êDFwÜ¿ïÿüÚ±'ÞUNASNone?ïk'',¯?œ'Í/iÚ?'½ºj?œ'Í/iÚ?íγ~"|ò?²Goß??±Šd7ÿr?²Goß??ìºs-õ?¥ÀºsB'®?¿,fWÑ?¥ÀºsB'®?í¯zþ	A?•˜iøF?²"(Hl?•˜iøF?í™ûWŠç‹?¸ô"¤ío?³0%B^é'?¸ô"¤ío?å4õãúï?Ï{ ê}¯%?՗Ö8
!?Ï{ ê}¯%?â÷ìb`¿«?¸>ñ1¤öl?Ú';>€ª?¸>ñ1¤öl?áïĜã·0?»IÊ8ó¼{?Ü vÆ8' ?»IÊ8ó¼{AGN4FGL J1748.2-1942¿Öæ½
¯Rá@ålÖÂðÀ9
‹ýáÀ;>–•[$@b'AcL«@-¢ÝåùÄ?ş£†ØL?¿=f<õÔ®?üT\É.²›?úÉ·0Ù;Æ?퍝aûÁ¿àfêþ<¿äSÇÝúœ"¿êHÒ!Š_¿Úý[?Á¶ï¿åës¶±•UNASNone?ïãbp7 €?móZJ7Rp?lÐž·?móZJ7Rp?êâŠ[¹T?ÙQy‰¹?Äu֑Æ°?ÙQy‰¹?ïLŸ¯¢?'ð*²Ì"š?–l
{Zî?'ð*²Ì"š?írKѲD?•`»ös‹Ô?´m¡s¹¨[?•`»ös‹Ô?ìÏ=Þe"?·¼θk^?¹†
AÒ ?·¼θk^?ΪdwC?ϱ,‹×Ã?èUfù"/?ϱ,‹×Ã?êÇïÔu?µ#ÇAÆ?ÇåÀà@®,?µ#ÇAÆ?Ýù˜Â?¼€0ÚñÜ.?ás3öžû?¼€0ÚñÜ.MIXED4FGL J1748.3-2906?ïŒïícEJ¿ãW;P8&¸À8+Apã—êÀ9Äöæ{Ê|@­õ«"A;@ý%àdYF?¿Ÿ©¾×ý?ԉƒâM<Ÿ@E¿9fS?üóâہñ\?ŃÁ–ò,?â<AßÉSÆ¿áÿÊñ*z'¿åž¯ƒêY¿ë˜ÂÚÄ¿ïÿÙi"A'UNASNone?§!ïZÞ?»XéXsµ?îïOb?»XéXsµ?²ŠQ總?¹bï¯L?í®¼5ÐÇX?¹bï¯L?Àž5Í8ÏÍ?ªãM[—D?ëØrŒ±Ì
?ªãM[—D?©`ïØ5MÏ?"‡%þ¶7?îiña.C?"‡%þ¶7?,HÂÃ\×?¿Ë­¤? ÞÙ?¿Ë­¤?€F'/ÏèÁ?•%ñžkÐ?ï¾å»RžU?•%ñžkÐ?¨"7GËãÇ?ŸÆ F'¬~?î}܋uƒT?ŸÆ F'¬~?MBÑ÷øn²?B]ûKÇ7?ïø¯K²…ú?B]ûKÇ7PSR4FGL J1748.4+1601¿ïÍÒèMd@4û3ÚøßzÀ:ÐðŽrôêÀ<K¡qÕ/r@Ɛ'ˆ(-@?']<9?ÒJ2žb×?Ù¦%ä@0ó@Àa"V!@Gœ¡¶Ê?émjf¦'G?ïý%?T©¦¿ç	¦ý…Qc¿äX,²²%¿ïþ\ý1§¿"É*gøUUNASNone?ïG33×?›£iÜO'3?—™£†Œ?›£iÜO'3?ìQE…[¡?Àv²Ü-4c?½uÓ×-"ù?Àv²Ü-4c?îOúœÇ?š`>Ž­?¯>*ýÂ~Ž?š`>Ž­?í%'D§È?–uJÖ½ç?¶ÖÅݺóÁ?–uJÖ½ç?îeº;r?®+âhÒí?®©¤_¸zÅ?®+âhÒí?ÝPÚD§?ÒsWXµ†?áW'ÿݬ?ÒsWXµ†?êÁÒ°''Ê?¬+×ûþ3?Äøµ=¹ôÙ?¬+×ûþ3?áYûTä?¼¬ÁHÇ?ÜýMæ	V7?¼¬ÁHÇMIXED4FGL J1749.0-2119?颢éñÃ@
0d‰Ø[À9…
a'ÏÀ:­y×\rÈ@»˜•±ƒ@<ó~}×?ÓÂìCŠ™L?ß¡2À¹o@ÛÐüv<?übJG¡Õ'¿à+"H×à¿âØÂ!y¿ëðÞ¤æ¿ëF®::Žq¿àÿñ½GÌ¿ïãtÿ†]}UNASNone?è?Ͻ†Í?ÑaªÑ
°C?ÏûÁ	äÊ?ÑaªÑ
°C?А<ËYÒ|?ÊuÜ2í`?ç·ášSÂ?ÊuÜ2í`?æ…fX?µ5%óŽë[?ÒõáÑõ3Q?µ5%óŽë[?äV%–gŠÿ?ºžr,©g?×S´Ó0ê?ºžr,©g?åe‡nHÞ?Ñ¡[«ˆ•¡?ÕÑ4ñ#nD?Ñ¡[«ˆ•¡?'¤éó"?¦µƒ£ õ?ïw÷â"ø4?¦µƒ£ õ?àÛgšC
?º
®ëÌ}ƒ?ßàI0Ëyæ?º
®ëÌ}ƒ?ŸÿÓà<k@?ž$%7í¹?ï`¹dv?ž$%7í¹MIXED4FGL J1749.6-3143c?ïã\]pjïÀn²Ð¢DcÀ:ÔK3ÛÀ<j¦gv@`ÆyvŽ}@åF
¦L0?Ðô»¾²'Ê?ïr7Pþ@ù?R%g@=‰"~¿Öy>‡$L?ï5ÞUö¿¹_ò.+¿ÜB‡d
¿ïßëìd?ê:#aÔÜUNASNone2FGL J1749.7-3134c?èàœän?ÉN÷8""?̹"nH?ÉN÷8""?ä¡uk<#?Ì­
_-j?Ö½)‡ãº?Ì­
_-j?àœ '-ä?³¡ÀM›;?ÞÇ¿ó±¤9?³¡ÀM›;?âÍÇÔÈø5?¸•¶öÊî?ÚdpVn—?¸•¶öÊî?֐Ùål´g?ÑYµPa?䷓
I¥Í?ÑYµPa?¿w"_mÏ?ÂÓo"®a8?ì1
"F?ÂÓo"®a8?ÄeìÁ½WÂ?°LBýðJ?êæ"ϐª?°LBýðJ?¼r@Aíñ?¬¿D "J?ìq·÷Â]¢?¬¿D "J MIXED4FGL J1749.8-0303¿à"ˆˆODa@(q[Ývh<À9.¨mqóbÀ;\ý#¬­s@·"CñòK@FC´g?¸¥.ßL½Y?Ñv°@O%'@}"Ó8÷˜@2A~$ž?ﹺAn_¿á"¹"K‰¿æŠ"XŸÔ¿çu –
¿ïþ@½Šd¿ïç0ž-}UNASNone3FGL J1749.7-0305?ín†®/}Ç?±eQJÚˑ?´‹Ê_øÇ?±eQJÚˑ?×ݳÞ`À?ːfMï?äv&Ï ?ːfMï?êйÁà¾?­:x¸'à ?Ä¿ýø}?­:x¸'à ?äfÑw;?¬p¬'H0S?×2]ɉô?¬p¬'H0S?تxLu'?É=Ÿñh?ãªÃÙÅ>õ?É=Ÿñh?«Î:žØ	ü?»pc¢3='?îCV;º°?»pc¢3='?Þ+.Ò{bw?µz»ã|ƒã?àêh–ÂNÅ?µz»ã|ƒã?µÏûK7‡?›žšˆ¢"x?íFžû/?›žšˆ¢"xMIXED4FGL J1750.0-3849?ï¿ÿª£4ÖÀz)³únÀ:FdÆSÀ<ø´²#Ô@ÝâF܈W@Xô›Gïƒ?ËJ}|­z¢?êÁLÁN¿V@ÍäKjb@šº†N8G?ìP¾´[<¿ÛÝÉtR¸4¿àÃ?O¡(¿ëúç\›Š¿ïþ'Ý¿áŠ¯ñʳUNASNone?χ0Yþ½Ï?ÐtGB½G|?è3é€PŒ?ÐtGB½G|?Ԟ:^†Ú5?Èö\¾î?å°âм'å?Èö\¾î?Û_D<ߞ%?´	"–°¹¤?âP]á0î?´	"–°¹¤?ÙÔU+M?±#˜¨±N?ãóüUjY?±#˜¨±N?Á÷%¾p?Ð$÷ËS?ë'?6y¤?Ð$÷ËS?­O\Jãæà?¹6¶ægšÇ?î+
;(†B?¹6¶ægšÇ?·fÜLlv=?¥›]ÑÝÑÚ?í$v›¬ˆ?¥›]ÑÝÑÚ?š†ß}ŠŒ?"xÄ*YÍ?ï+ÉêpL?"xÄ*YÍPSR4FGL J1750.0-3347¿Î׀7¦hÀ
™ÔttFÀ9Åét£@À;HöHÇ/@\ÜÇÁ @}N?(3ü?Ëøg…JW<?ÑUA8Úg@†&oÖQ±@¿"²²oS?ïüë¾TŽù¿è–µ¹ŠÑ¿É!"ßù$o¿åÞjNRsj¿é±y?%3¿ä¢W
--UNASNone?ïŸ<	¬?vp.B0ó?ˆ0ø³j$?vp.B0ó?ï`d]'om?"
‰a?"ótRù|L?"
‰a?î¦`Rú?–z'›¸'°?¥™þ?Úã?–z'›¸'°?ï;Ån(?z™ú¸¦xÈ?˜‡]òÊ9?z™ú¸¦xÈ?î'>c	‡
?§@|	ûQQ?¦ÜËj?§@|	ûQQ?ì{Ú0ãw´?Á<ãŽ@†?¼!.xäB_?Á<ãŽ@†?æÂ/»iM?µ<•")ÜÖ?Ò{¡Ü‰-f?µ<•")ÜÖ?ê¸Rl^x?®J
/ñÄ°?ÇѶN† ?®J
/ñÄ°	AGN4FGL J1750.4-1721¿ÞGž`cÿ@	$kðÀ:òÕuûÀ;¶၏¸@¤X[¶µ@ 6^`Þg?ÉϚ‡€<{?×ý¾¼éªÔ@»A®@ñ@…šPΤ"?îðÉ@Ñ+¿ãÁ9»ãp}¿â=d_%)…¿è_‹*ì¿ïÿÿ" 5•?ïÿû-2h2UNASNone?ãÁ˜NÖ?Ëð‡¸¬Ày?Ø|ÏcÕèT?Ëð‡¸¬Ày?䶶àÒ=?Ϙך!?×ޒ'>[…?Ϙך!?èÔÙôR¢º?¯eïU`¯?̬˜.µu?¯eïU`¯?ê8"ž7&?§µÂ¦'V?DZ‡³#j?§µÂ¦'V?Ç[Ÿ'E×?Æ®J@@
?ê)nŠ;?Æ®J@@
?­C ´X?¼¥ÏªD.?î.ÆõÎ?¼¥ÏªD.?Öà"ñW×¾?ºVV8pß¼?äî‡T!?ºVV8pß¼?É
›fš¶?´閠Û?é½Y&YRy?´閠ÛMIXED4FGL J1750.6-1906¿íkcϙl@Q€Ø´À9lm½r¼¶À;	:×lc@"!"9Å@þ7"«üs?É·¸=žœ
?ÌϞxÑx@}£!ØG?÷ô›ï	?ì4јäh¿ä×ø¿Äс¿é8Ï>ìúÀ¿ã»?Ï¿ì^ý¼Xá¿ïý‡ŸñøUUNASNone?äP2¹4?ÐÉyí=?×_›úz˜?ÐÉyí=?Í°Ž†H·‡?ŀrIQ5Z?è"Ü^mÒ?ŀrIQ5Z?éêK;eå?¯æ;ný?ÈVÓ–hj?¯æ;ný?ÚE¯¸¦
|?²:
Ô™¬?âÝ(#¬úÂ?²:
Ô™¬?ÁA{?¼X‹?ÃfÆÚ*¿'?믡0éÝ?ÃfÆÚ*¿'?–¦X>¼p?«Äγ`÷?ïJÍ=àá,?«Äγ`÷?דvLëôŽ?º"ȁ0?ä6Dي¹?º"ȁ0?šR•î?…"P¿Ý'p?ï/%]˜É?…"P¿Ý'pMIXED4FGL J1750.8-4405¿ÓCè*SïÀ!Jæ…Ûv´À:gþÓ°ÝÀ;àZ›W	@öä¡TÎä@Ò	Å{Ÿ´?Ðúk _pÿ?Ú?B5.µö@ž$»¡+^?ú¸`ygu¿Ø-³Âd¾ñ?ïÏ¡ýÁ6¿ÑµA*l»¿ä;ñb®K¿ïÿà?Æ>"?ïúñm–UNASNone?ïG2X?¢'®'—´í?ŸW`"5?¢'®'—´í?ííwþÉ?³W¼‰ÆƒV?°"@
h¾?³W¼‰ÆƒV?ëUwdKÀ.?¦¨Û9£Äÿ?ª"nÐÿH?¦¨Û9£Äÿ?íôÇđ¦?—>ޟù~2?°YÇë%MN?—>ޟù~2?è3$œ0f"?ÅmÒŒY?Ï3m>e°?ÅmÒŒY?áß1(lá?Ò+Nè›_l?ÜA¯'ö>?Ò+Nè›_l?åB¹^8£?¶Ðãž$·¨?ÕzCŽ¹Û?¶Ðãž$·¨?áÍnõÎp2?½ºÒEÔî?Üe"c›?½ºÒEÔîAGN4FGL J1750.8-1246¿Ù2"%°‹@å$9›,AÀ:€T–ZIøÀ;©Äÿxñƒ@2ް@º<÷T?ÖVԍ‹n^?ã<¥7\ @"ª^ã»&?÷y¿¹†?ïÿÁ¡u†¿à}i[
¿Ø|1©Æ7‡¿å@p"|ח¿ïì[rí]f¿ïäu_þmYUNASNone?ä1'.]?ÌÆBÑÙŠ?ם±Ï£õF?ÌÆBÑÙŠ?ÇÎ	Uò®f?Á±··U°û?ê}ªƒTf?Á±··U°û?襎ψ‹L?®eO_¶¼?ÍiÄÁÝÒÑ?®eO_¶¼?Öåüå´?±¶ÎŸ?ä÷%ÿ?±¶ÎŸ?Öñdþÿœ?̎òýõ
?äò‡M€€2?̎òýõ
?•À¿zB?«"¾€_µ?ïW1úî.?«"¾€_µ?ØV"G8ß×?º¹ê?ãÔîÜc?º¹ê? ËÉS±Ýý?Œ‰è¯Rÿ±?îóCjÒ ?Œ‰è¯Rÿ±MIXED4FGL J1750.9-3301?ß|0®"ÉdÀ¡f>ù:À9º:NÀ;9=e¼{@Æ<幃@–õw/?Éú»¡ w?ƹ«R5Ø?þ%½ÿªo«@v:2€Û³¿ë<":µ´?ïñ@x@.¿æo;At"|¿äf†a®pÁ¿è›
²ái¿ä5M>ÍPUNASNone?ïúOb†¢?P3¬ô?FÂw#e<•?P3¬ô?ïŽQL"îB?–`ÛK»vU?Œk­߉?–`ÛK»vU?ïhóÇÀüè?Œ8z¢?'á‡("ó?Œ8z¢?«áð ?sñ6­òœ?ŒÔùÅgù?sñ6­òœ?ïÄi{f;?ƒH Fø³?}ËBbíâN?ƒH Fø³?ì¹oÍ9Ñ?Ã"ràa
?º4–1t?Ã"ràa
?êäâUA9?²Js˜Ë_Ý?Älv«'û?²Js˜Ë_Ý?ë—VæÁ•Œ?°u[\–/·?Á¢¤dù©Ð?°u[\–/·AGN4FGL J1750.9-2655¿åý|ô?"¤ßʚ1À9)LøW>À:ªo ¡Ë—@Ýèuõ¥‰?ÿe©Oð?Ϧ-ü'6?áÅ»ámÛ@ÛxFbºà?üAmwþ?ïþµ}$îÍ?è­½¨l›4¿Öàæ?³¢¿ìzD5ë¿è¥Ùä"s¿î|¯þàÆ)UNASNone?㸹í"?Òì«ÚŽ×I?؎Œ%Î×Ð?Òì«ÚŽ×I?Æ{¢bÀêk?Å0v"/"?êagOÅe?Å0v"/"?âKÝ  ?µÌøjm-Á?ÛhD{ɾ¿?µÌøjm-Á?׉CÝǾ=?²QPóú?ä;^ â?²QPóú?ÝŠ,q×?ҋœi5VW?á@:éÇ?ҋœi5VW?Þl=ˆ$;?¤SN¡§?Oß?¤SN¡§?Ԇwvë?¶('A}ó?å¼ñtÄDŠ?¶('A}ó?­†]ÎM'"?œ¦ÿ\ܒ?î'š"Ön·?œ¦ÿ\ܒ
MIXED4FGL J1751.1-3455¿ì­ó·X'‰ÀUiR‹¾À9ø'õ:ª À;i²KAFò@_fPÁäf@ÿ#a.?Ê´®ÈÕÇG?¶)vpõ‹ˆ?ñÛCˆ×?÷WdZÈx?ïŒ$Ñp |¿ÞâšÎÍÙ¿ì{´ÚgÀ¿ÔBe"oä¿ê±ó˜°Ý¿ðUNASNone?ïì¾g@?fö!¸'?cü=P·[?fö!¸'?îêî«[å?«vŽS…m?¡QSEĨ?«vŽS…m?î½gÊÈf?•¥ŽÍì:.?¤)ƒVî ?•¥ŽÍì:.?ï0"Ä
Þ?|®æöÚ=?™íg|/S?|®æöÚ=?ï¾Tý}"?ˆÍ\׫ÔÙ?€jÀ³yí"?ˆÍ\׫ÔÙ?ê½<áÝ«?È,1n.~:?Džx‰T?È,1n.~:?ìUlÑíü{?¨§«Tâ.?½T™p)?¨§«Tâ.?èÒÊ®2ª?°É7Ĝº?Ì´ÕG£5W?°É7ĜºAGN4FGL J1751.1+0109¿ÑÏ}T?"@+ÙØ@žUÁÀ:E,YûÀ;°"L*zþ@ë"Ò/bC@œ'W…øÓ?Ԁr¡]2`?è*±^Ý0@Yàâi?ùøYMN<y¿åÚâ9E›ì¿Ý¿‹0JJ§¿èK"¾h…û¿ìœ.¿†S¿ÞÞõöÕ_¿ïó"כ\èUNASNone?íçÐÞ=}?¶cj¶τ?°Áyû?¶cj¶τ?ÖÆ!x†à–?θIär?äœïC¼µ?θIär?ìÓnZ.?¤óՓ.–L?¿_1d.?¤óՓ.–L?æ!eÎ]?¶‡ðyb2?Ó½øÅ4cE?¶‡ðyb2?éèë]Jw·?Æ´5oñ2?È\RŠÖ!#?Æ´5oñ2?¢Hg`­?´¥ß7³uŽ?îÛyŠk??´¥ß7³uŽ?âæíå¡/?·)©1£L?Ú2$4½¡â?·)©1£L?±ÖdïüyN?©¦Ä.Ör·?íÅ3bí¶?©¦Ä.Ör·MIXED4FGL J1752.0+3606?àóm@:î®ÀrKwÀ;nƒÚ³ìÀ<ÎI2xù@ ICF¦­~?þâ¿b€þ˜?ÐÂHyìU(?Â+ÍxÄ6ü?ó¨(Ãm¨z@»Ã>-¸?ېR.9#? El¿ÐZakTã¿È(aP¿íXØãÀ¯?À[˜·§wUNASNone?ïùh6Ó¯H?B€ÁÂ]?J_$¯íÿ?B€ÁÂ]?ïé;¿?hőZ:?fÄàz?Àl?hőZ:?ïŽÊØËÈ?Í`Òà?ŒMJlF?Í`Òà?ïÈ8¦Ã+l?aTg}–?{㬣9¾?aTg}–?ïížS	3Ó?``·ª@¥Ë?ba­,fþ?``·ª@¥Ë?C'¥.?¬–¹yå?‡Ÿo–´b?¬–¹yå?ïwÈB=V?ñ'c{`°?'÷³-Óô?ñ'c{`°?ï<ðÑc?‹ˆ87n?˜aåßSžI?‹ˆ87nAGN4FGL J1752.3-2914?ìR×ãk¿öž²r®sEÀ93âÏòÀ:N:†
˛@ÊØ"ì>,@zªÁ	J,?Ïfކ]§¦?×Jë I÷p@	wß 'á?þZ2H|›‡?ê,n¾#¼ž?ѺÔýÐ
¿åøÙÀ¦"ê¿ê7ÀÌ
Š,¿é¾u†"Ú¿ÆÌÉ\Tê"UNASNone?ã¿}zÃÚO?Ó¿ƒÛcµÔ?؁
xKc?Ó¿ƒÛcµÔ?Ððß	ÕÃ?Êô÷B[ù?燐{}ž?Êô÷B[ù?âÌÏä%ÑB?µß]v$_á?Úf`7´]{?µß]v$_á?ÝÊ\ȶpH?µç?¸ÔQ¹?áћ¤ÇÜ?µç?¸ÔQ¹?ÙóÏ;x7Z?Ј·¾6 À?ãbCäS?Ј·¾6 À?™¡þځ?±¸OÒ­?ï2÷Ðêc?±¸OÒ­?Ï~g¡½?µ\£ó¼Z!?è |fב?µ\£ó¼Z!?—½b
Ë¡}?ŠZ-­i-Œ?ïBïȜ´?ŠZ-­i-ŒMIXED4FGL J1752.3-3139?îË^"'À ]ˆ¿À9¡w·ÒjÀ;HóŽØu@DPó7š¡@õö&bjX?Îê—Ä'P?ÐY0ó½Ò^@uH#…@F?ðèҁӿìTS^¡Ëí?ïÜùjºˆý¿è–"ì"¿æ•BA˜ü'¿é7zàÆÔ»¿ÞR†à"d©UNASNone?ïÖÀH¯ò!?}S)WC?tŸÛ£7{º?}S)WC?ãñń{q³?Í0Æ8?Øt÷	š?Í0Æ8?ëãAŽÖ&?¨Fðí1p?ÀrùǬ§h?¨Fðí1p?èL¾ºîÜu?°
ŽÜ¯Ìj?ÎÍDŽ-?°
ŽÜ¯Ìj?íЅ»¸Ÿ¼?½eMÀ/ãü?±{Ò";#?½eMÀ/ãü?ÂÊŠ<Q?ÈõkΈd?ëMxù]pì?ÈõkΈd?ßGè´+b§?º/IïA?à\¥êN­?º/IïA?»ájÇ&Î?«&_9H
?ìœcÒ§&?«&_9H
MIXED4FGL J1752.7-3040?Ùg#~ùôèÀÅ«ÀãŠ~À9¶4EêPÀ;?ª9ú͑@؂Žs@–üõ‰"?Íi#šŽâ?âAº°j–@¥ò`L–?÷IŸsxGº?ï!FÁÛW)¿×Ï?"ª¤Ú¿ÞïåÿÏ®¿é¦2Ï`%¿ê€™'ódç¿ïö×B®\UNASNone?ê.k)Ó?Ç­} ®z–?ÇGæS[œ´?Ç­} ®z–?Ö@?Ðà?Êä~ý—?äßàpÀ?Êä~ý—?å²M—ãa?±–ÑQçŠ[?ԛdÐ9=ä?±–ÑQçŠ[?ØÁäÿý?¯Ò ÂÊî»?ãŸ
€~A?¯Ò ÂÊî»?à"ýÞÆ'?ӈ"ÛGA'?ßÚöBs²?ӈ"ÛGA'?ªãï§à]?·éLüû?îQÎÐ÷Ê?·éLüû?ı!øš¨Z?±þˆ"Z¦?êÓ·ÙUê?±þˆ"Z¦?™o1´?†!§a®?ï4†vôu€?†!§a®MIXED4FGL J1752.8-4449?ûÞàBóÀ"¡ÿ´€¥­À:9·	ìèÌÀ;éBí»YÞ@—M;@3ÁÎl	?Ç·&'?Ù_™ãÁZÿ@çń/_@KÐÈ:?íÚò)}§Ì?ì,â·Ý!¿Ù( ú"¿ã	Áv,'¿ëÜ>"Ë¿ïû¬áxUNASNone?áO°ÍEv?Ì©loÛì?Ý`üžeu?Ì©loÛì?æ«m¤yi?Å뚇¹?Ò©%Ô·
.?Å뚇¹?çñ#íšù?²fBúŒ"?Ð˸$Ê?²fBúŒ"?é5-Ϋ…?§`eŸ°Î®?Ë+‡HÅQê?§`eŸ°Î®?ÍÎM˜½&?ΕÛqÞÈ+?èŒl™þ·?ΕÛqÞÈ+?ÊIxŠç`]?ÇÞ'.(m™?ém¡ÝF'é?ÇÞ'.(m™?ÆcM«‹´?µÄBÐw5È?êg,U?µÄBÐw5È?ѐ绲ë?±ü²QÆÀ?çs7Œ"&Š?±ü²QÆÀMIXED4FGL J1753.8-2538¿é÷'HD‡?À?^¥&ë|À7´ªÄdHÀ:L$BÕg¦@þ¿e @ìÊì"?®c_/n
?Ô/ÆÂÃÖ@#š {5?øƤfý5?áÔS»d?Ù0W¶ :ž¿Ò•ŸäâBU¿â€Õ}uv¥¿ék¡~•\H¿ì¡¶hÝ9,UNASNone?V®'QçHb?ƒK©ÂHÉÏ?ïô¨·!rt?ƒK©ÂHÉÏ?¢wòdh?«=žO™—×?îÖ(e\Ú?«=žO™—×?¼:jõlS:?§ùÞãÈ?ìx²¡Ru™?§ùÞãÈ?cCŽê¥æ?T3î•,¡?ïì¼q4ö'?T3î•,¡?Uý,Œ3(C?`̪û…3¾?ïõiŒ‹"?`̪û…3¾?k»…Ç'?9—»Dýr?ïäDzÙ:?9—»Dýr?±`PÎ?ªëø%ßñ>?íÓõýaƒí?ªëø%ßñ>>úb(J¹eI>ô	(ü*?ïÿË;Ê}ß>ô	(ü*PSR4FGL J1753.9+2443?î'Gœ\þš@7û¨'j©À:2@h¥ÛÇÀ<[š'Í¥:@҉¹ý'=@ÅΞ^$y?Á"K©¡¤€?¶@+"-t?õbØ<l˜@
ÒÐ]t$?í˜ø‰éù-¿ç$‰¿ß~Q€ž¡¿â7 €=¨¿áXK»À5¿ïÿ¬ÞoâfUNASNone?ïü†iÍ4b?1ZO|k?;̱ZýJ?1ZO|k?ïéŽÇâ	þ?sôJç`?fq7ú:Í?sôJç`?ïìGçJQˆ?eÛ(ÞF?c¸ò'—Ï?eÛ(ÞF?ïøóf0?1ûö±Û‹0?L2gþ-^?1ûö±Û‹0?ïùÃ(;æê?Ck› P?Hó^'Wb?Ck› P?ï%ÙóÏ?"êpZ‰x?ˆ¶‰†ªhD?"êpZ‰x?ïæjÒ¶Ã?qð^cÃâÙ?i•-·
ìÔ?qð^cÃâÙ?ïð#qPM?I®|	ÿ ?_¹Jm&i?I®|	ÿ AGN4FGL J1754.1-4333¿ì'Ö_À!ϪŠ'¥aÀ:åªô4ð£À<Taä ¦i@!®ˆ Ø?áÔ"°Õ?Ú衾V?èçԐ­?þHż7SS@ª¥¼'—ó?ïù
ãˆÐô¿è¤±ÅàI¿î½_œr½?Ë®¿Æ~ÿå?Á4Æ[C¿í¥qß@lØUNASNone?ïù!ŠÐdB?N¨.ðßë?KyÕ[&f?N¨.ðßë?ïærU»{õ?|XҕÀÇ]?iªK;6?|XҕÀÇ]?ïðÌÂw?‰Ç5KŒ?æ`ÑäÕ?‰Ç5KŒ?ïþÒ¸
ù?c¿Ž5Æ©?"Ô|Ò5,ã?c¿Ž5Æ©?ïñd'û6[?pC'¿ðæ?]6ù¬é—?pC'¿ðæ?ïg…Q=¤?©ÊmQ0,?"\4 }€?©ÊmQ0,?ïow€®ÕÛ?'›+;®\?'äýÚ²?'›+;®\?ïþuoýÐ?-ºçxCæc?(¯æÝé»?-ºçxCæcAGN4FGL J1754.3-4443¿¬ÔìQ³À"ûR†µ'GÀ:x.åƙÀ;Ý Y§;@NµÖ\@Ðä¤Yæü?È;>"õó?×Wôž"}@‹š°@2+5㼨?ïý˜F³B¸¿àžÜd…¿áø#'¬?¿ç²ñYt¿ï='á>sÙ¿ÕyF<û3UNASNone2FGL J1753.8-4446?æ27|™?ÉMnÝ¥¯?Óõ›ó'Î?ÉMnÝ¥¯?è º[lH?ÃЧJºÁæ?Í}'NÝÅ?ÃЧJºÁæ?é½ümì1?¬Ròµýmù?ÉIøO:?¬Ròµýmù?ë[RÖ*ˆY? ¹ñg†®?'´§Uޞ? ¹ñg†®?Ô<ɬœo?ˀ¿€çyª?åá›~©±È?ˀ¿€çyª?Ư>5^ c?Ç.%0ªÜ|?êT0r¨Wç?Ç.%0ªÜ|?Ï:2Éße3?·Rw7,"?è1sMˆ&³?·Rw7,"?Ë÷@`9Èñ?­D0‡b?é/çñÄ?­D0‡bMIXED4FGL J1754.3-2915?è~­|ûSH¿üÙ`sÞ.À:<Ñ®³ÝÀ;Ï!CF¦­@V'ýž%ð@•§Yu½?ֆm'dsÈ?ïâp"&ñ[@c§@KIª?ýž€ÌC:?í«j¿îþ@5û?çÕk׿o¿ê¥_Ù.…¿íÛÇ4ÝW¿éñ\~†ÝUNASNone?à ®šBó?Ñ¿œß/Œ?ß¾¢Ëz?Ñ¿œß/Œ?ąOµñ`?ÅÊØ(ÔD?êÞ¬:Rƒ¨?ÅÊØ(ÔD?âÊë€cŠ
?´¬"¾ˆj?Új(ÿ8ëë?´¬"¾ˆj?¨¥¬ ª¦y?˜ÌêrÝ¿¥?îu¥=ç—(?˜ÌêrÝ¿¥?ÕÖd–hÉ?Ó¾çÓ±­?åòʹ˜?Ó¾çÓ±­?"55'»(?«ú‹·XÇA?ïfW.Sê'?«ú‹·XÇA?Ðr"b¶êŸ?´'¢…· §?çƽԊ±?´'¢…· §?o=ºÜn…6?l¶M™
ßt?ïàÂE	ts?l¶M™
ßtMIXED4FGL J1754.3-3236?îMK°¶hÀðƒB?@À:ðéÇ´À;}ƒvA¥½@þŽøœ@·†ªØ?Óý31…´
?çÜÄA
Š@~}ÖÅt@7§î&!?í Ɋ"-?ìT4ÀQn¿ä3¬Õ¶€Z¿îF—> Y¿íõ~†mÿïÉ$i¢UNASNone?鹃Âud?Æ»ÿõï?É•ðö*r?Æ»ÿõï?×ô'
A2¶?ͮȝñ Ÿ?äìzßf¥?ͮȝñ Ÿ?å°+^±?±®fþÑQ£?ԟ©õBð?±®fþÑQ£?Պ߰1ê?±iéóa&°?å:'ç
ø?±iéóa&°?Øhžl´&?Ò•ï•ú~?ãË°Éû¥í?Ò•ï•ú~?±6"ŽMÊ´?¼}Qö~S?íÙ;®_ù?¼}Qö~S?Èè¡"¾µ¢?²ÛCØt?éÅ×·PR˜?²ÛCØt?–¯i¥¹w?ƒ€yxla?ïJ‡4‰–ä?ƒ€yxlaMIXED4FGL J1754.6-2933?ìZ\áh¡eÀœ˜†À9<;¨LºÄÀ:ѕç]qË@ƒÅ[¿Cw@á';×F£?ÇFŠ¡Y,?Ý°å:¬Ï@¬$=Ìê)@Õú¿ïàk]¾L?ïÚ¶š[`y¿à4v)R	¿æÉúŠu9h¿ìÏÝ=]X¡¿ïÿC*!<UNASNone2FGL J1754.1-2930?áó<Ëbi'?Ò8	,Š³´?܆i;,ý?Ò8	,Š³´?Ï/ )"Š?Ëþkf'–?è47ÛõšÝ?Ëþkf'–?يÌåÔä&?±àTN?ã:™í?±àTN?àèý‡ª®À?´Ó¿iPÀQ?Þ.𪢀?´Ó¿iPÀQ?˼=é´‡?ͧ¸M0V×?éð…¹'Þ?ͧ¸M0V×?™í¼ƒöK?±#VC+?ï0'Ëãn?±#VC+?Är~ál?­
s÷lµ??êã`zǤø?­
s÷lµ??ª:=^Gm"?œ
v0*?î\\*H?œ
v0*MIXED4FGL J1754.8-3200?ï¼î…À
*s±éÀ:€aº/;À<AÎm¶¼À@zS¶xM@XÜ}Cø}?Ò	}!"Î~?ïö@líüÈ=@4¿ÆÔæ!?í+ž{ÝÇ¿Ô5edd¯?Úø¦¥×¿ß½Á+®Ús¿ïýÝ¡s²?î¢ÊšÃeEUNASNone?ë~VSŠ†?qÚ&ÁO?¦±ÉÕæ?qÚ&ÁO?ꍫÃà?Æ°s¥¿?ÅËýPðÒ?Æ°s¥¿?æ↊ž) ?±äQôuz"?Ò:òêí¿?±äQôuz"?æë·úéÑÑ?·†'@ɏO?Ò(
,\]?·†'@ɏO?åÖ
3ð?Ífº-Q¶›?ÔSÁãå˜ ?Ífº-Q¶›?ÔÇ\Xy}?ÐÌñ=x7?åœQÓÃrA?ÐÌñ=x7?Í}'
Dr?´N2𛝦?è» ›|®ã?´N2𛝦?ÐÝ)
6ìž?¿T®Bž
B?ç'kyd‰±?¿T®Bž
BMIXED4FGL J1755.3-3937?ïð#®ÛËÀ žý†¨üÀ:Y‰SÑ8lÀ;5^†ž@'êF/dG@bû…Fü>?ÚâLÒ?Þ]C½oÑ@
S½Ö.u@ÚÊö†?ÖªtÞ#aY¿Ð4à²\Þþ¿æ<˘fÙ¿æÎG P¿í9Ž—¿ïû
¢ò)UNASNone?햳òF•!?ÆUŠ–F}é?³J`lˆû?ÆUŠ–F}é?ëí{¨ÜÓ?º¾a¶9Ÿ?ÀJ_茶?º¾a¶9Ÿ?ìµÚ»U‰¨?¢ˆoÍ-ÊÝ?ºQ*%S²Á?¢ˆoÍ-ÊÝ?í":åâ¦?•Iw?³Þ(Ï3Ö?•Iw?ê/'HKü¶?Ù1ÝÑ4™?ÇCbÞÐ
'?Ù1ÝÑ4™?×)<I‡]'?ÐÞüÊÁYÒ?äkaÛ<Q??ÐÞüÊÁYÒ?á'ûI¯Bñ?¹í‰"¶?Üú	l¡z?¹í‰"¶?Õæ.ǂyÜ?¹£'¦óÉ?åèœ>Ã?¹£'¦óÉMIXED4FGL J1755.5-3734¿Èi8}ÊÜÀÂu%F
¦À:3qxéêÀ;´Ç%Ãß@àÃEJ7@¹}£~?Æda¾áҘ?´¥sl‰@0?ðËoÕzñ8@å½ïD¿í
Û¢R¦?ïâN>Qtg¿ëô…þ²"'¿ÙÕp_c'Ì¿àÍ]ìDaY¿å3TÁ"tŸUNASNone?ïúè‰@Ûè?Aõ‹ˆåçX?D]Ú©"?Aõ‹ˆåçX?ïÐ1#lj?…|¦³wU?wçnG1?…|¦³wU?aû}?‰uùåi&?g¬B°Ø?‰uùåi&?ïì¿Ìî?M}$ßò?cÿ@Zf?M}$ßò?ïÆX™ý ?'3³pŽ=/?|óÓ¸€ß?'3³pŽ=/?ò_ÐÂ?·¸Ó}kÛ?¦—ÀÙ'Ú?·¸Ó}kÛ?î+ãb‡Öñ?£œþ¨—,?­AÉÖ¦©ó?£œþ¨—,?ï6òQZl?Ž>rþæš?™!µÛJp?Ž>rþæšAGN4FGL J1755.6-2050¿ÑÞÝN,ç@'¹"ËÜãÀ9£B,Ë:&À:èî4%¡z@-=¹Ic@$ ]Øù+?Ã0ÞÖÏ/¿ŠSa?Ͻ‡?Ç×[†Žz?ý£øJÛ?îœÂþí±I¿á±—¢H"Ä¿ë7Rè`¸¿æd¿1ٖà¿ïÿþó…õ?ïÿùŸé"ÚUNASNone?î'=•ëF?¶Å¶zàLÛ?¦ì&®ed¦?¶Å¶zàLÛ?îñNU×%?®¿ÃÌ^m? ë®–¦¬?®¿ÃÌ^m?ìùxQui?§ÁÈ_EXü?¿ 4=tT¼?§ÁÈ_EXü?ïU*Gny?€Ð˜=Àž?•Z·røá?€Ð˜=Àž?äÇ𷍠g?Ìhg›MV~?Öpä¿2?Ìhg›MV~?åЩÛÜ	V?Ñý·½éQŠ?Ô^¬HGíU?Ñý·½éQŠ?ëC¯´&ý_?«.öÁ›?ÂñA/d
…?«.öÁ›?éI"nr'?¶a»³1?ÊÛvF5÷ç?¶a»³1AGN4FGL J1755.9-4009?셕²ž<À^[ÕêÀ:'ci[ä,À;±£_9M@/ðÚs(—?üè˜`´v?ÛúgVPo?ä%+¾IÒ1@!='AŽ@@¡~O'7Ë¿ïÿñh?ïþ¦>½·¿ÝÇv¡œó@¿â¥ýàÀõ~¿îßô╋î¿ïÃÆ^‰UNASNone?ïœ1*í?—J*';5½?ˆÿsÃ:4¬?—J*';5½?îÒ³1<°?§éžù+¯Ä?¢ÞDÑ7·õ?§éžù+¯Ä?덐¸ä&t?¦ä$)Æq?Áɽof.?¦ä$)Æq?î¾ÈË
á?‡\5`	*?¤sLÄLø?‡\5`	*?í,i$(JÄ?ºTþýÿþ0?¶œ¶ß™Ý?ºTþýÿþ0?êº]«Ï?ÊdEqEµ?Çó™‰PÄ?ÊdEqEµ?äï$ .š?¹ÃcÚÅß?Ö!϶¿¢Ë?¹ÃcÚÅß?é"Μ݋?²×¯`_¤?ɬǍŒ‰Õ?²×¯`_¤AGN4FGL J1755.9+0953¿Þsñ¶®[@0Åè´k­À;\Þê¸À<·k;¸=@"6°î[¾?úA
a'Ï@ƒû¶Å$?ïEj7¬>¸@¡¥×•~?û´Ê­7Ü¿îÖ¾ˆfko¿ïÿë<ú\R?ïû!ô›?ïšT	lL¿Ýº7~œh+¿ïþ"?½…1UNASNone?ïuK{Jñb?³xZ8?'V'zi½?³xZ8?çk°tžÛ?ÔA¥ÂîÉ?ÑÇ(ŸÂJ?ÔA¥ÂîÉ?î2Q0¾Ñ?Ÿ²Üßà?¬Úí®ó?Ÿ²Üßà?ëŒómlâN?¾üA~ê0?ÁÌ2JLvÉ?¾üA~ê0?ïùæ"ûÓ?Ê½lÌJá?ˆ†W'o%?Ê½lÌJá?áÀì"hWW?ל
êEÐç?Ü~&×/QQ?ל
êEÐç?ît6.ÿá'?¡3"ÿla?¨¼'Jö?¡3"ÿla?á|(oŠÒV?Óf}®½©U?ݯ ê[S?Óf}®½©UAGN4FGL J1756.3+0236¿éP²7Ó´{@*áŒâÑñÐÀ:#}At>–À;ž³ì+6å@‰Àë,ß@¥½"J¥@?Óm©PÆÂ?Õ
ßâ©-
?ðßXÀ‹v@ÒU%v\?ïïB¾¤Ø¿è=-rH¿ìRþtå…*¿äÏ/!}¿ëðžc,ö?·ºú½Jù£UNASNone?í9ê(l¦?¹Äz-m¡n?¶0®½èåN?¹Äz-m¡n?ï'R/ÞÑ?¤g"óCcj?›¹þþs?¤g"óCcj?ìøB*·?¥<cø;Õ2?»?EîªK?¥<cø;Õ2?ïLhtP¹?||"Ïÿ*?–rñƒRã?||"Ïÿ*?èé|vÚ8+?ÆtÖê ß?ÌZ$—R?ÆtÖê ß?éEÌÄO‹ë?É|Ï´]À%?ÊèÌîÁÐV?É|Ï´]À%?ä·{x,©?½"v€›?֑	¦Ä®?½"v€›?è"]ƒÐ?³*î0ÃÃï?Ͳ‹­ó˜¾?³*î0ÃÃïAGN4FGL J1756.6-2352?é":ÑHm¾?ÝÙÓÛߺ:À8"d鎤sÀ:/4q÷"!@ҝ{PƒP@
×^÷\?Ør³üœHK?Śx§0°ø@'Í|õôä@"\d"ä×?íQ`_¼(:¿í?½ÅGó¿Ì7¤/¿èpó‹(¿åôÑÞ¯xS¿ä@GƒLP;UNASNone?؋ϿÎë?ÓÆNsD_?㺠Šw?ÓÆNsD_?âyE]¤˜?ÏaÁäÄî»?ÛÏ
uD¶Ï?ÏaÁäÄî»?ß oÍ©|Í?ºÄ®ù²?à/È+Aš?ºÄ®ù²?埔áµ"r?³°´LÕ?ÔÀÖ<•»?³°´LÕ?Ò-Aat98?Ι×''?æé_OEãd?Ι×''?¹"ö£M?õȈ^L«?ì܍aIhv?õȈ^L«?ÙÒu0ŒBw?½
1\C?ãÅg¹ÞÅ?½
1\C?ºÿWŸµM»?¬R‰IFCQ?ì 	VI?¬R‰IFCQMIXED4FGL J1757.1-1926¿ïêë¥øD@Ķ¦ڝÀ9±RÝóe¾À:þ»dÅ|v@9Xo­·ß@6¡|¼ê?Ñ"0?ÙÛ¡¦ÙH@Ž¨¿§J\@Ç²0¿;?ïñ1Ñ3cÛ¿åÏ®&ïX¿çÓû_‡O¿èÃ^¿ìr±˜"à¿ïÿï¤h)µUNASNone?åCûÑX]ö?Ȥ؂ô¢»?Õx]OD?Ȥ؂ô¢»?Õi†Gh…Œ?ÉBú8ôEë?åK<ÜK½:?ÉBú8ôEë?ç²9ËÓ¨‰?²Yk'wA•?ЛŒhX®î?²Yk'wA•?åßÅæ?°Ì"7;?ÔAît3Ðß?°Ì"7;?ÒÓÉçÑF??ÉQ›h¦²‡?æ–\à?ÉQ›h¦²‡?–ý
³ý?¨dŽÚTÈû?ïH')?¨dŽÚTÈû?Õeé…âz?¸èsћÚ?åM=Ã?¸èsћÚ?¶ÌÁ냂g?¢†"¿v?P?í&gÂÔGã?¢†"¿v?P
MIXED4FGL J1757.1-3554¿ï#æÕó£7Àˆ.D¶é6À:aÀ¥wnÀ<|Dôü—@º÷dP±@/¦¥ñ—?Ìr‰µJúû?á§ZS<=@áè¢ì(³@:ßý¥?ïþ¾°nÈ¿å$@ò8— ¿Þ`\̉°î¿ç¸A¥f׿﵂˜Ì@¿îñ›MοìUNASNone?ëÊ¿«?ù?¾!–P?ÀÕSó?¾!–P?ì{ð"ôU?¸È£.3‹?¼ {Ø_õU?¸È£.3‹?èr…U>÷?±Ms/GwU?Î7åê«%?±Ms/GwU?í.ûÕ?"#æ"=?·&‹xý>p?"#æ"=?åÝC¥Ï»r?Ë;eØ'?ÔEx´`‰?Ë;eØ'?Úv`7ÏX?ÐeÑÃÆX?âÄÏùäT?ÐeÑÃÆX?Î<!#;Cx?µ¶±ˆ0?èp÷·1/"?µ¶±ˆ0?àÿ·ý™?³ÿ.Ko?ÞȐÍù?³ÿ.KoMIXED4FGL J1757.1-2848c?Ĝ§±ñeoÀßOC427À9¸™9!ŠÀ;!-w1@
2AEÆ@ðÛâêE"?ɇø‡eºo?Ò¡ÿěÐÖ@	Gcä«æ£@«.4ä³?ïã²,¿Üáàš´÷™¿äµü¦¯,¿ç´<G®ë:¿î2BÝË!Ò¿ïÕ ÞœØéUNASNone?êìâuß?Ä\žÅ5Ò?ÄOŒv+¼ƒ?Ä\žÅ5Ò?áÀm\?ÍZ£fÄQ ?Ü%ÏóGá?ÍZ£fÄQ ?çjêöiºj?²B;ÃÁ?Ñ**,‹,?²B;ÃÁ?çÁèÚÁÏe?©±wN¦?Ð|.J|a6?©±wN¦?ՀTùÎÛ?Ì|¢"«e?å?øՃ"?Ì|¢"«e?·súbW?Â"­qgÌ?íq€Üðm?Â"­qgÌ?ÒVI©¨k«?¹3¥H·$?æÔÛ++Ê+?¹3¥H·$?ĆÊR&Æò?©à¬µw"?êÞMkvND?©à¬µw"(MIXED4FGL J1757.4-3125?à­÷"'äÃÀ«ºÅcLÀ9xäû—»sÀ;‹w·Òj@²:öËú@›´áô|>?ÀÁ_Eà´á?ÕàèãƒÈw@ߒޔum@_5¤ ?ïš½ÐZ¡¿ŽWÚÌ-¯U¿â«)yv
£¿æª)¿l ¿îà÷Ií¿ïòè ¹UNASNone3FGL J1757.8-3126?⾄A¥?ÌZµÅÁ ?ڂ÷|ßà·?ÌZµÅÁ ?ä'}ߺ÷I?Ê¿pÝ|Œ?ÖÛ@Šo?Ê¿pÝ|Œ?á¼ÑË¡¡?µ(€X;;§?܆]Þh¼¾?µ(€X;;§?ç?·a;ë?ªNŽB?ÑÁ€'=ˆ)?ªNŽB?ÁߐÿŸ»?ÆڍŽ¸-ó?ëˆ;›À?ÆڍŽ¸-ó?Âðö`R?Ɣ\eS
f?ëCÂ\'ëy?Ɣ\eS
f?¼¸wãï?°SËÔá5"?ìhñŸ?°SËÔá5"?À¯¾©Ég"?£ån´j`?ëÔU¦?£ån´j`MIXED4FGL J1757.6-2731¿ê¶I-¤·¿øÐÒëʾÖÀ:	 »aj~À:úÑ9C­@†"'&3@mâÀT?ÝlRƒÛlM?àëEþçÒ@
x¡UO¾?ÿm>ô‡|?ïó$Oj¡_¿¼‡!F÷‹<¿ÝA"Šfð¿ã¾¹ä¾¿ìÆÝ»²s¿ïïë€:ÕUNASNone?æ']ÙW¨;?ϐ¡©Ä›6?ÒÝDMP¯Š?ϐ¡©Ä›6?ÖÐÇÆÜ%Ž?Ì¡þë¢?䗜'í9?Ì¡þë¢?åµ-ýFñ?³1ääd¦Å?Õ̕¤r?³1ääd¦Å?äÚ#`h†¸?³*Ã@s?ÖK¹?.ò?³*Ã@s?Ø©aª·Ež?Òb·ç?ã«O*¤]1?Òb·ç?¢®ÄP¶Ø˜?´»œÙØš?îÕ»ÍÆ?´»œÙØš?ՐýªT?¶oEá"Õ?å7þ*Õõ?¶oEá"Õ?ÀåUÔ6½E?¬…ËVÓ]?ëƪŠòP¯?¬…ËVÓ]	MIXED4FGL J1757.7-6032?ïý¼ãd'¥À1/ס<%JÀ:4Ú§€âéÀ<iË@ے@œÝ‰š?ú
¦ç_ö
?ÆÍÆó?Û]õ¿	j¸@³·õfI?÷Ïxw
#?ï×táSl¿âYbqå ¿Ó™û꽿͝CÝ¥b%¿ì}y¼"€¿ïÿßéà
UNASNone3FGL J1757.7-6030?´3;Ç7~Ë?À	rûE–?íy˜‡BKv?À	rûE–?ÕÕÚ10Ç?È[^oñÿ?å|'çg?È[^oñÿ?Òõl±·¦(?±t
[ØÞ?æ…I§$,ì?±t
[ØÞ?ß÷â{¥?µ·óėÐë?àxŽöÂ-?µ·óėÐë?£Ïê˜?£k^Yò¾?îÃ^É ?£k^Yò¾?µŒÆÙÍú?»t'0ŽÏ?íNg$¸'N?»t'0ŽÏ?Ï._)íJ'?·@{½	?è4h5"­`?·@{½	?µù€CŽ?¡ëJ•"@-?í^€ÐL¬?¡ëJ•"@-PSR4FGL J1758.0-2953?ë Hj|öÀ0ÄÃéÏÀ:uK8¶ÈÀ<Tlô!-@-¡"¹ï@ÞZCBtð?Ò¥î[è´	?ïçùÿ4þå@U ÃÄæ?ýYnîöt¿îë\‡Ê?ï8tP3ôú?èëÏO^¿ã ž9%¿ï1…ý¿ïþ·á-VûUNASNone?Õpp(d«¯?Í­i«ÑeÊ?åGÇëͪ)?Í­i«ÑeÊ?—ãämÓ?Ä,…ˆÚHz?ëZ:†ä‹?Ä,…ˆÚHz?Ù·ýºÖU?³}kN?ã¼""Õ?³}kN?«"'¿hý?–•Êª?îM×ßO†P?–•Êª?ÅA3£'??ËÁ"ªÏÍ?꯳;×°?ËÁ"ªÏÍ?'WÅC(9?¨)Ú½ýÜL?ïmAÕôyö?¨)Ú½ýÜL?Ã:™m¾Ž?«Wѕ;à?ë1yÙ¤\?«Wѕ;à?|͈³'?tè¢S>þ?ïÆdï 'O?tè¢S>þPSR4FGL J1758.5-3219?îÂÞjÀÀv–€àe0À:|r®sErÀ<
ÿ"Év@{Ý/E'Ü@
õ ¨ìô?ÕA[j	?îL%þpÛ@hò'hûl@Ñð~Ø£?ïÌù"@F¿àÓm›
à¿ÒjwØ~±·¿êìgpQ¢¿ïãh¬'Ä?íρ'¼±UNASNone?ì"êœÛ1X?Á˜ˆººä?»`«&u=?Á˜ˆººä?ë0ۄÂê?­òÁ,õ?Ã?"'ìôW?­òÁ,õ?éLÞ_Ç;?®~ª»6¼?ÊÏ̆€ã?®~ª»6¼?ê~îð/ŸÍ?¬Oe˜áö?ÆD?A€Ë?¬Oe˜áö?æ0Ekõr?ÑL8K9Ô?ӟu÷(?ÑL8K9Ô?ΨèùËè?Í壱(4/?èUÅÁ ?Í壱(4/?њ"Da™?·ª¹_Ç5À?ç2½ÝÏ14?·ª¹_Ç5À?ѱ#²üZô?¼>ñÁ'¡?ç'n&Ò†?¼>ñÁ'¡	MIXED4FGL J1758.7-4109?Ýԛ
ô«À õìløÀ9w)@k*À;´è·äÞ<@´ËLD&K@³|™®'?´ËÞæ)ë?ÄxÑ¢õbî@
Õ¥á¦x¥@–'(6*?Œa¢²¿Ô±d ·¿ä€¿B Ž€¿àø>•'ø¿ê«ïxÉ?¿ïòÔÔK4UNASNone3FGL J1758.8-4108?î/ÙL•y?±ÁuИ‡–?­k4ss?±ÁuИ‡–?í
)<þý»?´ðÿÎU-Ç?·–¶¾7¨?´ðÿÎU-Ç?íâ{ìp½>? iZ_~?°ì Uý? iZ_~?íÀþ6ô€<?unMCS?±øH[þ?unMCS?àn¯`*b?̆]g9J$?ß÷"¡?«<?̆]g9J$?ÞÙà= ?Î×{ž?à"Àá0?Î×{ž?ßØ^œ©ªš?½Z1,{f±?àб«*³?½Z1,{f±?â¤fÒ?²ŠêؐS?Ûз2[ÇÒ?²ŠêؐSMIXED4FGL J1758.8-2326?ïø1q‰|?ÐÏÝMx"À9B£©½ÔÀ:"Õ¿º•"@ "»tৠ@Ö«ÃgÉ=?̕͜«qÞ?ÛG>©@åídòÈà?ûºouá\¿Üçòº•=¿ì½FA­?«ƒ¾ÆÎu¿á'§àÚ¿é¡!ƒ†Ý¿ïÿúÁҝÇUNASNone?ÂE"…áßa?Ãrm…¿r?ën›‡ˆ(?Ãrm…¿r?ɁFBޛ?Æ2y$?{?韮ozÈY?Æ2y$?{?ߛ)€pÂz?¶½IC?à2k?ǞÃ?¶½IC?Ú³bËô'?µ…«LGÌà?â¦9Nš¿?µ…«LGÌà?¯©³1å
2?»•¡+M$?îdÌïm?»•¡+M$?Štfj~_=?›`]Îóœ?ï–.fVƒ?›`]Îóœ?Í=•ŒÄŸ?´B=`Íd?谚œÎØ@?´B=`Íd?¢gMæ¥?•:¢j??îً!ºB?•:¢j?PSR4FGL J1759.0-0107?绘gÈï¦@&7ÏÃøõÀ9Û÷÷oÀ;c§¹íÍ@ó!6Ü`@ƒÂ‡çÀ?ÍÃք´?Äï@£3?òãII.?þ\ÀJ]qJ¿³G'±Ê½Ô¿æ‹¨ñf¿ë··¶ùҿ絟=Ø©¿ïÿòɶ—×?î*éŸ¡UNASNone?ïIs̀v³? ®'`¢??–цgZ#¯? ®'`¢??îKâD`àž?³îOh…ëá?«AÛ¶'Z#?³îOh…ëá?í³ª™h"µ?¡¸¯¦È?²b«4»b[?¡¸¯¦È?ï6u>+Æ?ƒ]wO¥Ù;?™=qV'¹E?ƒ]wO¥Ù;?êйGx©N?×òÙ?ĽâZÉ?×òÙ?á"…òY
?ÓbHûœ?ÝþöôMí?ÓbHûœ?ç'^šü+p?¶z/CU?ÐûBÊ©?¶z/CU?äùŽ]¯ó?½EO¼#û?ÖãEè ?½EO¼#ûAGN4FGL J1759.2-0243?è¨~4í"@$¢hn~bÜÀ:cÒuðGÀ;ì†<Ń,@f°@O%'@Ó€™?Õól^MW?ïTów[0@ÀŸÀ$GÞ?ÿ=±nwí?îU€šÅÄ¿â;`"¾ŽF¿ãÝï3ÿáÍ¿ïH­M«"¿ïÿXJ?ïý÷ý}ÚUNASNone?â˜ïà¨?ÏõgÀP	?ÚÎ ?̯Ø?ÏõgÀP	?ËX<.Pí¦?Æo:\?é)ðôkė?Æo:\?å™,±ä¿?²g$ü`ª?Ôͦœ6ò?²g$ü`ª?Óۀªñkú?´.(IÁ°?æ?ª‡J?´.(IÁ°?қiøí;?Ð[êiUp?æ²K‰wc?Ð[êiUp?"Åzóçý?¥¢´¶ßõ?ïaÔ(`Ç@?¥¢´¶ßõ?ЄÅ"D´¡?µ´x¯H•a?罝nÝ¥¯?µ´x¯H•a?wL£ØÈë?"•ë,*Î?ï|Ešá9¹?"•ë,*ÎMIXED4FGL J1759.6-1850¿ãÊo7#
@îÒ£¦bÖÀ9'ÿ#a.À:ãóbb˧@•o¨@Ö¥†6æF?Õ/š¢X/?áþ¡ñ@XÈh¹ý½@{èP¶Ñ¹¿é¶V˜í!?ïûáÝÖ	Œ¿æ!['—¿é¶ˆRIxð¿éÀ¤ ^¿®<kb›øçUNASNone?ìOÄsz*?ÃTN‰–[?½Ügä.­?ÃTN‰–[?ÚÚ%¢žGv?ξåxÀ01?â'í.°ÜE?ξåxÀ01?çþáÐr§?³y^㓢Z?ÑÆ<_±?³y^㓢Z?ã ¸¥Vï?µ˜ÇŠvC²?ؾŽµSÎ"?µ˜ÇŠvC²?ãl¨S?чÇ!ðžA?Ù&¯YýÕâ?чÇ!ðžA?ª8óñ¼¶Î?½"[£%?î\pÀÿ±s?½"[£%?ÕXVž`3?¸Î(þ?åSÔ°ñÏç?¸Î(þ?§gú.<¥ä?›8pJE?\å;â?›8pJEMIXED4FGL J1759.7-2354?î1Ƥ¦¿Åe¬­À8b¥)œ±À9™‡(}͋@ Ÿ:o°­@€ýÁ?ÎAN)Ø¢?΃*Ar>@€¦ƒŒçÚ?ûÞ?Þ½:3¿èÑÿ'›?çk<Žü‡¥¿Ö<×ÁóT÷¿áŽþµýþ¿êȸÀü4¿é–ƒ?4{UNASNone?È3–cò?Ï	Üàôª•?éú3g=?Ï	Üàôª•?À¤òñ­4Š?ÂC+¡¢U?ëÖÃC"²Þ?ÂC+¡¢U?ÓW·'…;O?²âÂ2 ?æT$l=bY?²âÂ2 ?È?´Eâb?±Æ€×é¦ñ?éðú®‡g?±Æ€×é¦ñ?ËúíBIaÚ?ÓÛf;&?éD¯m§Š?ÓÛf;&?"~¤Ã×?œÓ¹Á{b?ï®l¯t?œÓ¹Á{b?¿;êÅcÕp?¦¸ü}—ïñ?ì'§S…R?¦¸ü}—ïñ?w?d¬Ê?qÀ%bMǛ?ïсèՎ?qÀ%bMǛPSR4FGL J1759.8-1250¿ï¹ã¼Ó@5Ïò=À9¸Ÿb0wÀ;A;ʸ@ýz¤6@ÝâïN?ÉÌ7;*£m?̱8òÔõ@ùæ
‹t?õ©%Lj½?ïöBçÜÌ¿çÖòU'¿ãêÕ+@«¿Þ]¨[ý¿ìÓ~AÏX¿ïÿð懈öUNASNone?êû‰Ðë7?Â`:NŸ9?ÄÛ̼S$?Â`:NŸ9?Û¿fJ•X?ʎúQ'?â LÚµSð?ʎúQ'?ëÿþ2J€?¨ïþ¢>?À6Õÿü?¨ïþ¢>?äØQzÆð•?¯[9/Î.4?ÖO]
rÖ?¯[9/Î.4?ÜUÇKQ?É©Dm©b?áöÕZ1W?É©Dm©b?°R@¤ê?½W°^4Ç;?íþu·ù<S?½W°^4Ç;?à¿£¤4}5?º|WU?ހ¸·—–?º|WU?¾°îèß»?£¼éËxHm?ì)â"äi?£¼éËxHmMIXED4FGL J1800.1-0323?Ø£m$×·@#•¯)M×#À9r•Q5}À;3Íw·Ò@Še¹ä@A#ßYw?Å¡«¡Y¢?Æ»Jî:Ü@8'¹ÑG†?özՖ´¿ï˜Ô!Õ½·?ëJþ€ù势è–ý»'"¿æªÑù\¿êLŠÝ"T¿ïÿö$´ë/UNASNone?î¿ÀQ`½'?®+0Æ¡ƒ?¤úë«û•?®+0Æ¡ƒ?àm-ÜBqÑ?Ï#XRZ‹?ß%¤G{_?Ï#XRZ‹?íC/üo}?¢I8þÛ/?µæ‡d¶?¢I8þÛ/?çáÉaïou?­VN*?Ð<m<!!?­VN*?åó¢à¦Z?ÊæŽÙ¤Õ?Õðº>³M?ÊæŽÙ¤Õ?º—å¤ßóÆ?Åå=Ô?ì­Kd‡?Åå=Ô?â=㩙R2?º8øb/}¥?ۄ8¬Í[œ?º8øb/}¥?Ä`pÌ#+?±éççd¼?êçãÌ÷µ?±éççd¼MIXED4FGL J1800.2-2952?æ´þ«¯À	³åZbL%À:<†&öÀ;Ðכ\è8@ü±A%@Vî#^©Ú?Ò2B…Þ?éC´öl@©Ì1œZ>?ü°Rÿ?³«`Á`Ýæ?îtOȕ/¨¿áƒŠc›±¿ê0ô)2(q¿ìÀØ7d\¿Ý@*<•UNASNone3FGL J1800.0-2955?ۓ·Ûp?Ða5鵫?â6s¹$H?Ða5鵫?ÇnÁ(Ôµy?Æp–ôOT?ê$OµÊÒ¢?Æp–ôOT?â¡-jO?³­"~?Úz½¥+aò?³­"~?ÊSh·7?¦Úœ¦
ã€?ék%û'2?¦Úœ¦
ã€?ÉO·-(W7?̱·ü
àœ?é¬4µê2?̱·ü
àœ?•ŽÒAo¦?©?á,ÛI?ïS‹ñmôƒ?©?á,ÛI?ÀVá|öå?¨Éü<ö?ëÿêG ÂG?¨Éü<ö?ŒÇ!^–Ûœ?w€û<Ï"?ïŒãz…¤'?w€û<Ï"MIXED4FGL J1800.2-2403c?í""æE*¿Õ¾¤žvÀ9:G#«À:A>Ž±@"¾]ž@zÑî0Ë?Ð輁ûî#?¤8ût*b?çk;³´M?ü@°?è‡G½-óX?ëÍGF®Ê¿éö;ÏÆ|¿äûñþ_–é¿ãMÁÔÌ ¿ágÑ­ÝUNASNone1FGL J1800.5-2359c?ã>áٓ˜?ÕÇ¯÷æ?ق<LÙÄÏ?ÕÇ¯÷æ?è4«æÇI?Ïj	Lô"+?Ï-Pg˜âÝ?Ïj	Lô"+?ä5&:t?¶¹Kb­]ì?×Á•Ý³‹?¶¹Kb­]ì?ꉳaZ§°?³Å²àN?ÅÙ2z•a??³Å²àN?à¡KԌ+>?ÓC²öü?Þ½hV穃?ÓC²öü?ÚcQ$#ƒ?Õ]­³Ë?âÎWmòn>?Õ]­³Ë?姭D,é?½'þ.'l?Ô°¥w¦Þ.?½'þ.'l?ԗ,ràÙZ?Ä졶Û?å´iƏ"S?Ä졶Û0MIXED4FGL J1800.3-5237?Ô6"ñÀ,!ámmÁ¤À:óp–kðÀ<jm³aÁ¼@õ^£ylS?ó²õú:Ä?ÚsW%*ÜÍ?çZ)ûÒ@p¨ß‡ºt?ýÒv发X?ï«P°ò{³¿ìi¹Âƒó•¿"z±ÄU&o¿Ý#½¿"©@¿èW B•¦Æ¿ïÿ¬óéqHUNASNone?ïë=U€ò?fE•¬Á;ä?dªøý-n?fE•¬Á;ä?‹ž?Š\s'àmß?~ý3Lu+?Š\s'àmß?ïU\|=úH?‰ÝÊoëÄ?•TpsM?‰ÝÊoëÄ?ïcç"w–?z?ó`av?"ƒ
'?z?ó`av?ïx¼iÓ-d?—$î'hy›?èrÀré…?—$î'hy›?ï=/µ>) ?­rPځùç?˜Z	Q["?­rPځùç?î«»©.Ö?œ%è5ͱ?¥DEq|®¢?œ%è5ͱ?îИ$ q?•PmW{¥?¢öK*Cø?•PmW{¥AGN4FGL J1800.5-2910?¿‰òwÀÀ`¾¼hÑ{À9"ùdŒÀ;æA@9
6u@¨âù3?бuBø";?Ԕ@~Ë7 @]›¡±–?û÷Zþÿ$?àɀ2Wk?ìùŽâ0Œ:¿áÑ>vˆH¿ëGÁ	Ë¿ßÛÄhû¿ïþ)›Ú¼zUNASNone?î‹OÏÿË?³¬í'{¥%?§KâêK?³¬í'{¥%?ÙHÜ
˜«?Îï·ücÆ×?ã['ù3ªt?Îï·ücÆ×?轆D–÷˜?±¨zjQ?Í	æí¤!¢?±¨zjQ?áaÞÂ\u?·ƒ[ç'?Ý=ÊB{G?·ƒ[ç'?åõ@Å~?Íä;>½Ö?ÕÉÖ~u?Íä;>½Ö?°¸3ÕÈÞ|?¿¤pÉQÿ?íèù…+gQ?¿¤pÉQÿ?àôiHekâ?¸²y!yÒ?Þ-o5(<?¸²y!yÒ?­{ÎÑ?¡jO%Ãc6?î(C[ÝC?¡jO%Ãc6MIXED4FGL J1800.9-2407?íeÈm¯¿à]Ÿ¤u–À8DAYA»À9Îb뇢÷@ ì1"‡c·@Ĩm'K?ÂÓÝ7S(q?ÂÏڞF§"@
 ðbÔ
¯?úo·UlC?ïÿ&@±v¿ì§w¨®	"¿×
;&òˆ¿á¯`«;'¿æóû_‡O¿í¨]»WUNASNone?Ӛ¾GMòQ?Òî/SæÃ)?æ2 ÜY×?Òî/SæÃ)?Éîz˜2Ín?ÇŅ"ò¦Ú?é"aYóL¥?ÇŅ"ò¦Ú?ڐOú¥^Z?·8;dªÛ~?â·Ø­PÓ?·8;dªÛ~?ҍ"—'6?µ0ǸA΢?æ¹n´q>å?µ0ǸA΢?Ò¢²M€Í?Ӏ'÷?殦Ù?™??Ӏ'÷?']@¦M?¦û=x†y?ïuú¤\§?¦û=x†y?ۆ։ö¼?»×k‡ô'É?â<"»ð¢?»×k‡ô'É?-»ŸßÌ?"Êå;_{?ï~'#~€?"Êå;_{PSR4FGL J1801.0-2802¿é"	UÀº;<ìðYÀ:+PâÌÀ;¹ë1;â.@÷§kê4@Ôef—?Ìô¡}Ð<?ãÍ?ïXz@¢G²?ÿÝ#?_¿ÀçÉ'{Äò?﷙ÊAR¿Ýö5{âÏn¿ç5šìð¿ïâ&›u;ì?ê¯òkÂƺUNASNone?ÝÔÓX¤~F?ÎΧØ̊]?á–S­ÀÝ?ÎΧØ̊]?΃&ï
Ã?ÇÑ:@;§?èyŸ6D=O?ÇÑ:@;§?àùx"væ?²ß¦rۑ?Þ
÷È4?²ß¦rۑ?Ü>éÓKt¦?²
ޕ3?áà‹ZE­?²
ޕ3?Ñvø!Ö{?Ï"­ê^ƒ?çDƒï}Â?Ï"­ê^ƒ?'Ãî*5JÊ?¤ëÖó>?ïqàŽåOi?¤ëÖó>?¹=Bµ'€?¤KÂՊÞ?ìØW©xù€?¤KÂՊÞ?¤†´5bs¤?'t hç?¼e –?'t hçMIXED4FGL J1801.1-2626¿çE+øΪÀ¿û,0ªÂ¶ÉÀ:X`£®ÆRÀ<5ßüTz@ k\sÉPk@DR´Øº?ÒիÒ¼[?ïكÿÔa@þB҄?þ\×w¬	?îŠ<d4\ÿ?ÓÔ
c†7<?¶ûlâU°¿À]6fïMU¿ï€¤ ]Øù¿ïö-ƒÆÉ~UNASNone?½v–µ8±w?ÂÂ.ðŠË?ìQ-)XéÑ?ÂÂ.ðŠË?¸Ï838—?¾…`Ò}»Ã?ìæØÐ]?¾…`Ò}»Ã?ØC s	"[?²®5­Âä?ãÞoÆ{=Ó?²®5­Âä?Ÿê8Òá7?Š@ñ6äm¨?ï®+ª†?Š@ñ6äm¨?¤LPÕIaã?ÁˆvÀ´;?î»:ò«iâ?ÁˆvÀ´;?"#ô&(ª?–®žUÄlQ?ï¯p-î…?–®žUÄlQ?ÉÁF ' ?¸P܂]¤?鏮WÛwú?¸P܂]¤?e^ûì}ŸÇ?aqnÍÊ?ïê¡X:?aqnÍÊPSR4FGL J1801.4-4307¿ëµ!ÒJÀ#³y1DEªÀ:Tb(êÀ;ÛüwµCC@½±$¥¦Ã@œ˜D/ú?Ò§›ûH¶'?ÖáUðÍ]@UÆ2o?ýL…>õ?ïÿÕm…>™¿Û½?¼¥!¿å¤œâ¤O€¿èGGÝdI¬¿ïÿþÐñ?ïõv'[¸UNASNone?ï}ýù.nl?›DšcÃõ?@@Õ
ȁ?›DšcÃõ?礪T?¯Cç'ÅU…?¤Õ1L'Ã?¯Cç'ÅU…?í«nˆZ'?œ§ŸIù?²¤‹¿Ã"J?œ§ŸIù?ïV-­.Ä?~–uÜ%ßP?•>zMÉÃu?~–uÜ%ßP?îÒx¹¶UÎ?¦Á/Þ¦°?¢Øt`O $?¦Á/Þ¦°?äìáj=¶o?ÐáÈÎñ±?Ö&=+"""?ÐáÈÎñ±?çÕ&ˆ*?³XžÚ¼¬?ÐU²ï«ôæ?³XžÚ¼¬?è졾M¥r?µ™î¥.E?ÌMyÉj9?µ™î¥.EAGN4FGL J1801.6-2326?î°Tû¿Ô,™î˜ÏÀ6À.¬»µMÀ8óq}ñg@bQ#35â@IN…Ÿ?ºÍHÁºË?ÔiQÓ1jÜ@",pCß?ûøúJ3ß?¹Ëw7Dù¿çõYé€aº¿Ùk	ä/iû¿è\ƒ3&¿ê˜È]ý6L¿ïý ½é¨UNASNone0FGL J1801.6-2327?$6"yCá?A›59Ò¾?ïþ¼—†«?A›59Ò¾?¡='¾<?¨
ƒB"n?îì/7Èe¬?¨
ƒB"n?Ã+'ñÅæ»?­‰0º¹Î
?ë5CŽ†Q?­‰0º¹Î
?YœD¦n…l?N´]Û&Xk?ïó1ÝÀ?N´]Û&Xk?ô#ŒæǏ?Ԓmš& ??ë÷ÆN?Ԓmš& ??kMlØÀ~?€08ó·«Q?ïä²áX
ø?€08ó·«Q?¶oç2ó?ªñ½òêBÔ?í=R×â?ªñ½òêBÔ>×A±â©Z>Ö$©£Ým²?ïÿô_
Ä>Ö$©£Ým²PSR4FGL J1801.8-2358?ï€ä•Qœ'¿ãŠoŊ¹,À8''Œ6À9îC–Wź@!Í-Ŷ@e¦$ÂW(?¼"T=ïÐ?¢¨süüë?ñä¶Î]Ç@W``u?Áüža)?ê¶( Þ†¿äµešŽŒ¿åAÍÊùö¿ç™§ÜR{οݡ…Æ}þUNASNone?âv&]ô«?ÔΚ—£ÿ?Û³Eèª?ÔΚ—£ÿ?ë.ýã‰ì?Ål'AH°Ú?ÃGÄqØN?Ål'AH°Ú?ßÍÇiòž)?¹á¦3ìý«?àK°ì?¹á¦3ìý«?ê+l÷ø?±íjì¦ê?ÇROÌ#¸?±íjì¦ê?ÓS?Ó<$š¿	?æyòðÖtõ?Ó<$š¿	?à‡Fö‰‰¬?ԕJŠ?Þñrìì¨?ԕJŠ?â%
C$íË?Äà7?Ûµëy¶$j?Äà7?×?[¤ZV§?ÃýÞx×é?ä`R-ÒÔ¬?ÃýÞx×éMIXED4FGL J1802.1-2652¿ì3¼'Úø"ÀÛšþôgÀ9Ë
By!TÀ;U
×ÊVÑ@ù
ö¸®ˆ@c4ÅÚjD?Ì/ú;É°?ãA³ß@ñ@ûÍxÄ6ü?ö"Gx¯p?í¡ƒræ§i?ï5+ÆWgÆ¿Ü2+`ÖÚm¿éNÜd…¿í/êß‹4¿ïÿa>ß8àUNASNone?·.UíŒ$?¾É€}Úe?íš5‡«?¾É€}Úe?³ò0:ƒª1?ºb‹6:µÅ?큹øxú?ºb‹6:µÅ?ÕVq€(?±øv—¯Q?åT¸G?ëº?±øv—¯Q?ù1¸<z?…Šyr!?ï6r>,?…Šyr!?3´r°C?½9•H¸;×?ïg¡"®?½9•H¸;×?€üLe¸k?–>¶¥í/±?ï¼Îq_
?–>¶¥í/±?®e-˜sçŸ?œ_,v°ªe?î­&O†6?œ_,v°ªe?L"yù‹™N?Aæ')T?ïøÛ!_‡`?Aæ')TPSR4FGL J1802.4+3634?ïé_c›c@9
TûÚ×RÀ;®ÉÀ¨ÒÀ=L-·É/‰@<# –x}@©Ã}˜²?Ô¶Òd'O?ëÄ=aŠ^"@£ñb®K@k
>pN¿ï Å®?ïýáý¶y¤¿×6ÿ[x³¿æ`¾ø¿ë)ZÖ¯O¿ïÿô!O…úUNASNone?ßé[ðõC?Ð×^1tÓM?àRu‡…_?Ð×^1tÓM?á†'O?Ììõ>äu?ÜóÀû÷÷b?Ììõ>äu?æ"êÐ×Ï?´AõQêó?Óº*_òPa?´AõQêó?ákN˜‡œ?°ôÒˆ×?Ý)bÏØðÇ?°ôÒˆ×?ÃáãAOÍë?Ê W+"Š??ë‡/¬…?Ê W+"Š??ÀÅ"ñ%?žLß#3?ëΏ^úƒ·?žLß#3?ÎFc;¹"Œ?»ŒK£þˆ˜?èng1šÝ?»ŒK£þˆ˜?·"W¿¹Ò?¡Ç
°ý?íou?…?¡Ç
°ýMIXED4FGL J1802.4-3041?îQurÀ3YÀ+"¼ÃjMÀ9¢{oâæëÀ;ÍÑÑ‹è@dÓr®HR?üېIŽ¿K?À¡u´6S?Ö
´ôhó	@åB˜I@†â8™Ït?ﯦ¶¸ŽQ¿åé,êCÖ¿Öl^"9¬¿Óoô¤Ø$¿åÚpú>¿ë©ØÁw¯UNASNone3FGL J1802.4-3043?ã懈ŽÉ?͌ÞP¾ð|?Ø3úðîân?͌ÞP¾ð|?Ù_!?¸6?ÎÏòë¼É?ãPo`#ðå?ÎÏòë¼É?ãÃoæíµP?±ôŽ«3]?Øy 2$•a?±ôŽ«3]?åËm€zÓu?®»}ÛR?¡?Ôi$ÿ
Y?®»}ÛR?¡?à'²ž¥?蘘Ú?ÞÛúšÃîµ?蘘Ú?¬íîêà²S?¹àÅkô3³?î1!6wû?¹àÅkô3³?å'™;r>X?µXæqÊ®Ì?հ͉ƒO?µXæqÊ®Ì?Çõֆ^ÿ??°ƒAó¨IY?êŠ^h@0?°ƒAó¨IYMIXED4FGL J1803.1-2724¿ïÄ5a`ÃÀw_}>@À9m@wÏDÀ;÷¹à`þ@4úXKE¤@·Í+d2?Äé‡B©ó¯?ÐTÚ¢ÎL@Jd`Ò©@\+ž>nü?ßeˆÜ?Çõlh³ó¿ç'•`$¿çÁý &¼¿ã.ÕÖ`ÊE¿ïÿöàœjUNASNone3FGL J1803.1-2728?ê6Re?Åf|l?Ç&µû"Îm?Åf|l?à*>pº8‡?ͤêΞÕ?ß«ƒ‹Žò?ͤêΞÕ?ëN—v…î?¬@_b-u?ÂÅ£Î%èG?¬@_b-u?éÉ@{ζ?¦WèN|r"?ÈÚþÅ'Å?¦WèN|r"?ß1¾`p?ÎÚbIÿ±?àvøç ÏÈ?ÎÚbIÿ±?®fá¥;?º3±)ЀX?îé'å¬?º3±)ЀX?á
mâí²?¹?ñ¢81q?ÝÉå$:$?¹?ñ¢81q?È$éP]‡è?°ò6E!ÍN?éöÅ«èž?°ò6E!ÍNMIXED4FGL J1803.1-6708?ïÉsø†u6À4[çÈіÀ:èÅPØÀ<Rdë<#@ü:à>Å?þ߸Í;‡–?º†ÕFÃÞ½?Ð,âxY@|¶"‹ë[@à[8Šàï¿æË£¢1пۮ!æڕ¿ÝW˝>?¿à./ˆƒÇ ¿êÜV|E¿ïÿÿ&¦³UNASNone3FGL J1803.3-6706?îÞ¡)ʘ"?¢X¯zž°?¢ífƽ?¢X¯zž°?ïkè¿O>_?˜Dq(t.?''記?˜Dq(t.?ì"õQœ?ª‰ÛŸC>Ô?¿{`Uw£?ª‰ÛŸC>Ô?ïq5±N?s×ý¯")ç?'Ý<4"lH?s×ý¯")ç?ن¯QfÏî?ǔ€¦¿®?ã<¨WL˜	?ǔ€¦¿®?ìx´û?ËÅșè?¿_W$:X'?ËÅșè?Ô"•ùsk?·ÖÑÆLN9?åünµFJ?·ÖÑÆLN9?ëŽî«wp-?©x`#9{?ÁÄER"?N?©x`#9{MIXED4FGL J1803.3+2425?ïHi"lƒâ@4ðx…LÛ{À:SºÜ	€²À<
A¢a¿@#úVå@¾"[Có?Òñý=­àx?ä㼝ª R@™Ê&)_u@¢+'ôØ¿àí0_nO"¿æߝ‰é"¿ìùXç!â©¿äŒpPÊó¯¿ï½þž0§¿ïéÜ»WUNASNone?ë]òý–¡Ë?®2uü?ˆ4	¥xÔ?®2uü?è?¿™Äž?ʀrT
üË?χ˜íˆ?ʀrT
üË?챍Y?¥¡žՏ‹?¿Bs—ý7N?¥¡žՏ‹?éØä¨`±Ç?¬œ¥Cm~?Ȝm^}8æ?¬œ¥Cm~?ä ÉÙät?ͅëvÐR?Ö¿òlL7?ͅëvÐR?Ë2>Óû??ËäÆ#÷g;?é3~ðK0?ËäÆ#÷g;?åŀ¥Ú5?¶ƒ)"‹?Ôtþ´üK•?¶ƒ)"‹?Ç*¤ê쮦?±$ø'¿*?ê5VÅDÔW?±$ø'¿*MIXED4FGL J1803.5-1639?ïÇ_=äMX@,ئãÀ:"¿Z'ÈÀ;ß[.ú¿N@zƒEÅ1"?þ­<^Uí?ÙÓ»¾Ýuç?ïBR‡"Ä@¥b?8È?õ£Þ&;~?ïí(Œç°¿ç|˜×ÒºM¿à±Èà5j¿î'á@øÔ¿ïÿÅGMƒ?íaâ"oUNASNone?çaùf«'?Ñå"Õ©%?Ñ÷<
2©²?Ñå"Õ©%?ȑ2ó?ÇE"šè_a?éÛ¹»3Xƒ?ÇE"šè_a?å±Ø²h?±"æ\µ–?ԜOûڛ0?±"æ\µ–?ÓÈúÃU?¶øÙºkØ3?æûô'žU?¶øÙºkØ3?áЛ_±/Q?Ô²«¬tEU?Ü^É@¡]?Ô²«¬tEU?ƒÜ´ÅÌH?'o
&ë?ﰍ-xG?'o
&ë?Õ9È1ÌD«?µë$â[¬?åcçݪ?µë$â[¬?¢%'?}?š'ÒçNþ?îÝ®èî?š'ÒçNþ	MIXED4FGL J1803.7-3207?ÞÍ[Á–ÀâP.ì|•À:
5Ä+mÀ;ó`µL~@ŠŸþ…,@ù×Vé?ÌÍ£6{g?Üp¼`mþá@;=ïí™@ó
Ýԇ¿°žaÕ]-?—B&rþ¿æÛÆ/#Ùú¿åÚv»œ#¿ïü`Ÿ±?ïÖ¢
±nUNASNone?îàÿ†¢5?°oU9¢ ð?¡ÿ0x­?°oU9¢ ð?íí"ÕíÝ¿?µvp,Šbõ?°–éQlù
?µvp,Šbõ?ëâhžò?¦º#¯Î?Àv_"7ˆ?¦º#¯Î?ï.‹ž":?" òW
©Ø?š.Œ4 (|?" òW
©Ø?í$Èf-'ù?ºò:ÚòTq?¶Ù¼ÌÞò=?ºò:ÚòTq?۝ó‰,‰?эËzgOE?â1;iž»?эËzgOE?׿û#ˆ€?½c>åT>W?ä n;¿@?½c>åT>W?åÌ.áP?»øãc°J?ÕügÍ¢=`?»øãc°JMIXED4FGL J1803.8-2908¿Ðm…òü?	À[
Ø/×^À9··ä|À;UûKeY @X4Pi¥@(©6Ŏë?ÏLáÚûä'?íÕ€ÙÚ@Uí¡Xª¼@¢ŸÒ™?çˆ]‡º¿Á":šZ´¬¿èœRnM¿ìz¨<ʋª¿ïÿ¹ô'ô<¿ÞՋ¸/‡UNASNone?ÂeH,ó?˜͇ê?ëf¿íôÃ??˜͇ê?¹ËÆßÅDe?¿+͛ NÌ?ìƇ$Ws?¿+͛ NÌ?ᘬ7£R?³¸%ˆS4Ö?ÜÏ⧐¹\?³¸%ˆS4Ö?¬½Ïvþœ?'ÑÙV<?î4#ÔÌ?'ÑÙV<?Ðä Ç?ÑÎw'?獯œv~ô?ÑÎw'?ˆ%G7LŽ?V¢Ä¨ z?ïŸjâÞ^?V¢Ä¨ z?ͳ‹4sq‰?´ùÝs…€?è"2ã#ž?´ùÝs…€?QhhøӘ?@8"ÝÞC?ï÷}ːjO?@8"ÝÞCMIXED4FGL J1804.0-1124?­r/ûQ@r€Æ^À:)vþUÀ;ÇáR•Ï
@D•pÀ–@Ê)"]È2?Ñޘ\Þ|?èd÷eýŠÛ@•—'$@8 GÉa?ï69bwCƒ¿Þv¦…:g¿å
¾"Š"¿îp;Ñg¿ð?ïÿþˆ0»ŠUNASNone?å"™¯OJ?ÎÙµAڄµ?Õ»ÂÌ¡am?ÎÙµAڄµ?Þý¦BŽ3Ï?Ћºß˓M?à,Þ¸æ?Ћºß˓M?ç¬þâYã?²3ší±½µ?Ц;L9ó?²3ší±½µ?æ³÷úß
?±?Ë
¥?Ҙ
AÕì?±?Ë
¥?Øl^F¡ù?ÐQõiÓ?ãÉÐܯvƒ?ÐQõiÓ?Ÿ´£WªÙ)?±"ÎÆëïú?ïZåB©7?±"ÎÆëïú?Ñy¤.¦)?·\*ýák
?çC-謸k?·\*ýák
?¼6ÿa–ë?ªß`ª
$ï?ìy<`Í#?ªß`ª
$ïMIXED4FGL J1804.4-0852?æú_]Yó@ò[1~þ
À8ùg+ˆDÀ;	q(aH@~öº†ú@¼R?¼©HðÕ?ÁØQeMa³@›ð™Z¯y?ÿªñ=D"¿×
P`½§¿ápv̗¿èÆ6°–5¿à½!=èBõ¿éþ=½Ð°‡¿ïýtÀc‰UNASNone3FGL J1804.5-0850?ï(o+ˤ?Ÿ²$À'%?šòƒÐV?Ÿ²$À'%?äœúzb¥D?ËEV^¹ýE?ÖÆ:µw?ËEV^¹ýE?ì°"ɝ\6?§i¬Ñ?º~é³S?§i¬Ñ?ê00æ«?¤15ȍ?Ç?Ã?ìeU?¤15ȍ?ׁP‰Òž•?Ël5R0Ó?ä?W»°µ?Ël5R0Ó?ÆmáÖn?ˍ<ýŸí?ê}$‡¸Šd?ˍ<ýŸí?â•4ä§ù?º¾/™(c)?ÚՖ6°Å?º¾/™(c)?Ì qQHis?°Í½CG€?è×ã«­å£?°Í½CG€MIXED4FGL J1804.9-1745?èâÎfT%?ýjJ÷uÀ8ñOýnUHÀ:¥}§Ë‹"@© u@t@ë:Æ¥k_?Æׄ¶³…Ô?È#ë†Lá@›´&Ú@š€©•?è°×£Àd	¿Üúû´@å¿è·—{ž¿æÀҝòâ¿ïátYn0_¿ïʓ׸¹UNASNone?è0K¡p?É*ڟg?͋>Óáz??É*ڟg?âq†šZ×	?ÊE–(12¹?ÛòËJQï?ÊE–(12¹?çBª´ôéÌ?³úÓÅÍD»?Ñzª–,g?³úÓÅÍD»?çp-*–½­?«¬c1
û'?Ñ¥ªÒ"¥?«¬c1
û'?Ê:øê¦Á?ÂõmÕÆp'?éq{ÅVP?ÂõmÕÆp'?º´X¯Í?ÉZ<žð?ì©têü¦?ÉZ<žð?Ö7Ñ#YÝ}?¹j½´?äänSA?¹j½´?óàö- þ?¨³}Ò[?ëÂt·À?¨³}Ò[MIXED4FGL J1804.9-3001?Øk.Æ«ºGÀ½–ÁxôÀ:NBM'iÒÀ;Äq£±J@š&\`(@
r¡Þ¹?ÒËáÀNå?é¡Xª¼Í@XØ>?õ5ßðëåí?éŸåŽ?Š*©_Ù¿â©}g^ß¿ëY‡ZÒ´m¿ïíVy-?ìÐý³õeUNASNone?àš»½'_¸?Óy1¨!Od?Þʈ…±@?Óy1¨!Od?Ä}ïb+¡Í?ÅRbòØ>	?êà"'u?ÅRbòØ>	?â´(·ë?²ýÿjþ?Úz—Ù®)?²ýÿjþ?ÀIa!Fæ]?£<¯j3?ëí§·®Fi?£<¯j3?Õ¶¶j'!?ÓÙ,Ô@Ö×?å$ý¤Ê¾ï?ÓÙ,Ô@Ö×?•"&瘫?¨NâæG'?ïSÞÏXÃ;?¨NâæG'?ÁÁ
CGJ?©ÒNa¤ð?뻏½o..?©ÒNa¤ð?n©`µš$³?`IÇHý=?ïáVŸI?`IÇHý=	MIXED4FGL J1805.1-3618¿é;Ëfß÷¼ÀóÜìՁÀ:wè]À<Rµðè5@VðqB8?üç,å;Xœ?Äôe˜
Ma?çuÜ%/dr@Ÿñ=Å]m?ù·Ÿ•g¿ïøI©ƒò?ïÿߞ¶Žó¿¾í¼[t'¿ã؃ÿÿT4¿ïÿþR€ÖT¿ÞÛ^ºËmUNASNone?·j—K×1?¾ý¸}	–?ír­$CŠ?¾ý¸}	–?ȯP	ƒ?"${pŸá?éþÔ;«ýŸ?"${pŸá?Ï<†»gìñ?±iî
~?è0ÞQ&Ä?±iî
~?ŞøÑëù?§S¿v¡=?ê˜A˅»?§S¿v¡=? úùµ''?·ƒp¶)$ð?îðPdòH?·ƒp¶)$ð?£‰¦ÀM8?¬à³·çˆ?îÇe"Çam?¬à³·çˆ?§CᄩmX?˜4.´xó?î‹Áçìbê?˜4.´xó?…+IÛ2š?t–9!½Ÿ?ï«S¾¡™v?t–9!½ŸPSR4FGL J1805.7+3401¿ç69±bÊ6@7ª>iƒQÀ:A8æÑZÑÀ<?¨Ï—'h@p4Æ[D@…6…Î
º?¿m´¹Zª?Ó\K$Á€h@ûd8Š‹@óΆ‹Iö¿Ó˜dMk¿Óɏ*ªÎu¿ç
´¾¹
Ó¿è¬.È—‰¿ïüVB+ô{¿ïÿX°›>UNASNone3FGL J1805.9+3407?æÍÜÝ;â?È¢/óÁ?ÒdFE߈;?È¢/óÁ?èñg¿¬Ô?ÅF™Xç?Ì;ŽaL±?ÅF™Xç?ê[zXFú!?­M^+Õ'?ƒžä}?­M^+Õ'?ë8{=|Ñü?›åS7|Çe?Ã
¸?›åS7|Çe?Ê,bÁb­Â?ÄvãLƒ?étçO§T?ÄvãLƒ?ÍîðKÿÍ?Éq uÆ?è"Cøí
?Éq uÆ?Ö¨¡ù£Å?¸j½ˆ³¯?䫯{ƒ.?¸j½ˆ³¯?Ñ4³‡<°ò?¯ïËQèú?çe¦<a§‡?¯ïËQèúMIXED4FGL J1806.1-3344?ïÕ
_RåšÀÌ$·omÀ:KX+:@nÀ;©$7í­@*RÁ@|¦CÌ?Ë÷Ám9Í?ºÛ~K››?ôC‰!|QŠ?ü
zW_?ïè³}pn'¿¶1NA+™a¿ê-uïpeÄ¿Üú"[ADC¿ç©E©W|¿¿çh̽]nUNASNone?ïýx0	Õc?9c.E´$?4>~¸›~?9c.E´$?ïYpT§?¡¾oàÇ
?"ÝP=)?¡¾oàÇ
?ïhû8'?…øý®÷6É?ˆ»åÎðKT?…øý®÷6É?ï‡Vƒ&ª?p'i"÷?Ž*ŽIƒ?p'i"÷?ïõ"<kä?a©zÐ'?T׆ψë?a©zÐ'?ì½æµx•?Á[Z"`R?º ÊT;Z?Á[Z"`R?îFƒêÏ?£7"ا^o?«—ÎdÖ
?£7"ا^o?ëêÓ~Jf^?¥^³Iœ?ÀT²Öf‡?¥^³IœAGN4FGL J1806.2-1347¿ïV'Iµšp@ͨ_/:€À9d
`:Ó;À:¦R©@@P€u[KÖ@<ÿ?æ"&À´½?Ú|ûî"ˆ@Ô²ÄãÊ?@Jîí^Ù?Ý·äx:#¿Ì"è^x±¿ëêQBóH¿éªÞe{…¿éipafø2¿ïãý5Jd¨UNASNone?åOQÔUy§?ÒG|Ãls=?Õa\WU³?ÒG|Ãls=?ß[鉶:£?Ñ֎±M?àR*=b®?Ñ֎±M?æbkYóÅ?´¼/]Ë8?Ó;Ó)Lv?´¼/]Ë8?䡸ŽEÑ?º1;{?Ö¼ŽãÕt^?º1;{?Ä­®ñ¼è¡?Ê°ïæF4?êԔCÅØ?Ê°ïæF4?¾1"Y=«T?ÉIEKí?ì9Û´ØJ–?ÉIEKí?Û$~}ðN?»ŠtðdN?âmÀùÁÙ?»ŠtðdN?¦CÊw`s? ãñ—ÛŸ?σ¸? ãñ—ÛŸMIXED4FGL J1806.2-2126¿ê†–?›¿Ð)TÂÏóÉÀ7œ;
˜	wÀ9{ÛàfÅ@øùSéa-@¯R¹
x)?¹nV\ƒ?ÔfÏ­QÝB@œýÒ(V@‹Ù_'F—¿ëÀ³ï†59?äɂ—½¿çEfîVŠ¿æ;_ýk¦¿îCC¡•f"¿êÕ!Ð4`ZUNASNone?¤˜[/jjœ?·ðñ`;:O?î¶zLÄ¡'?·ðñ`;:O?¨/±:Îq¸?®Ë=,e¡‹?î}스?®Ë=,e¡‹?ÈU½¦îí?±–pZH/v?éꐿÖDE?±–pZH/v?©Xÿ¼'°?–
}{c $?îjp[µ?–
}{c $? 4ܚd­?Âì‰Loo?îü²6Y¿u?Âì‰Loo?q=ëE¥P?€œ"÷öB#?ïÝûƒ÷úV?€œ"÷öB#?¯×厴?¤¢¢èû`?°ÿ?¤¢¢èû`?C%&î3?;GڃW3?ïû<6ðŠ ?;GڃW3PSR4FGL J1806.9-2824¿î3,ÖÂÀQ1eәpÀ9×]	ÆR_À;i²lÏ64@ãÂh@>±Ä2ÊX?ɺwàŒGL?Æ"³‰.èK?ÿ9MÿgSÌ?þÒ&"©x4?ïøò?Mé¿â›`
†Ñ@¿éÖJêà¿æá@øÔ2¿æp,XN¿äiUßZ˜þUNASNone?ïeȐkâ@?¶§@'Cj?"Fí뤀?¶§@'Cj?ìJEH‰‡?½$ÑÎáœ?»}­Õ»³Ë?½$ÑÎáœ?9As?¡©}€H	»?¯ۄÏ?¡©}€H	»?í‡UÞ.?' (Ú֋?³ÅQ:v#?' (Ú֋?ë×po²H?Áà—@43Ê?À¢>A6ߙ?Áà—@43Ê?ØyÆr{Ú?Ò*=ôµÓ?ãÃ7œÆÂ?Ò*=ôµÓ?çø»ë©ó?¶@Žx×;?Ј(­ô?¶@Žx×;?ÞàìB?¶ðR_‰­‡?à‰òÿÞ¿?¶ðR_‰­‡MIXED4FGL J1808.1-1234¿Ým4Á0j@
7S½vÀ9—žþ]h'À; Y}I׺@9 M'Úä@A*¢jùs?Ëub'¬K?à™Ã‹«@çԝ{¦j@Xbz¥c¿ãæ5‰NÈ»¿ÕÉ^BÖiY¿å¸ßDž•'¿é"+Þ«¢¿ïwj·-ÿ¿ïÍî'Ò-UNASNone?Ý)æðï?É÷Nå…I?ákuŒý‡ˆ?É÷Nå…I?Å8­¬²6?ÂW:'âA?ê»qԔÓr?ÂW:'âA?ä¨yŸc?³Aó
Ù`?Ö¯Àá9Ê?³Aó
Ù`?ÞP6E®­I?² @+›¬?à×äÝ(©[?² @+›¬?·mÒý°˜?µ
–ýã:?íE PË}?µ
–ýã:?‰½VQ	L?–AãžL;*?
b«?–AãžL;*?­.gؒ?ªÁš(Zž#?ëT´f	Û\?ªÁš(Zž#?ÁßyÃS?‰îl
¾j¡?ï÷q;+¥?‰îl
¾j¡	MIXED4FGL J1808.2-2028e¿ì¯ÐÉl×*¿ÇN%ýÀŠŸÀ7»èc+HƒÀ9 »åô»ÿ@'p0?@Z"{$c?ŋ-ۅwN?àQµSGP@D¼­šØ^?íå¢^±‰?ïßï¿@P¿àö¨ž[¿àŠN½Ó4Æ¿êd†'UØ¿ð?ïõò`L–UNASNone3FGL J1809.2-2016c?Ãqpð?Ï)'…UêÃ?ë#£þCß ?Ï)'…UêÃ?¢Iä2k£l?§·Dë»|"?îÛa¼¢L
?§·Dë»|"?Ñ;³#GG?±(¦fuS?ç~b&n\]?±(¦fuS?{T'¡9%?iýQ"½$Û?ïÉW°Ò+˜?iýQ"½$Û?Ô›ŽÄÜò?ÙÁ¶ÛÁ(Ì?åÿ28'‡?ÙÁ¶ÛÁ(Ì?l·Ê—ø^"?z¢tp˜á?ïãH5'¢É?z¢tp˜á?´4cíú¿°?¢™¿¹{Ò­?íys'iãZ?¢™¿¹{Ò­?	y¹«®È?ÚÀôF³%?ïÿš r?ÚÀôF³%PSR4FGL J1808.2-1055?ê•ö–—(@¿ÂÀð À9 Ô ~$ÉÀ;"ËêN½Ó@¸Á'Z@@ÀA¤>?Ò;"ÀÊ5?éXV£zÃë@"XýÈ[@ëLk'?ïÅbu@ý¿jØ»dç؎¿éÍd1Xh¿ìõºAYç}¿ïÿÿÊPË?ïþÍeyUNASNone?Þh>*»ž?Ñg…JW<?àËàê¢0þ?Ñg…JW<?Ð]Jˆå?ÈØ+ra?çÿ÷QZ»?ÈØ+ra?æ™<löV?²k¨?Ò͇&Sß?²k¨?à  ­ù¼´?µBŸQö_?ß¾¾¤†™?µBŸQö_?ÉG™@G1²?Í	µáMã?鮯î3"?Í	µáMã?‹‹ªÀìï?š†T]ôS¯?ï'ÑU6'?š†T]ôS¯?ÓÕ|&T?»l²£ßK]?ætÁülÖ?»l²£ßK]? 
DW»[?¦q><ÃÙ?îÿ+ºv'Š?¦q><ÃÙMIXED4FGL J1808.2-3005?º Ïi›`Àd¤L{ÖÀ9âOOÉkïÀ;oÑEØQe@« ¸qÌ@É$¡ŸøX?̀–Rè/?ÑD¼@àÛwŠ{@žªfpwa¿å¶PôåË?ïø曪ëѿ僲ýmÔo¿äØ=‹ü£¿ë©n*¿ïï¢OJÀîUNASNone?ïG±'ù?—HÌí²E?Œ.¯LmÉ?—HÌí²E?ëôÑïã}?ÁšÛ°aÔ?À,»à@r?ÁšÛ°aÔ?í*xAw«?¡A=×¹ÖI?¶¬?†b6)?¡A=×¹ÖI?í,·ý÷€ï?–¥ÐŽÂ2ç?¶š@Œ*ˆ?–¥ÐŽÂ2ç?êò©>8†?Àq7>ŸfÒ?Ä5[ç®?Àq7>ŸfÒ?ޜ»`¶?Ô
Ô¨ÓF?à±÷"O¤ó?Ô
Ô¨ÓF?ã²~±¥™?¸
o_v?Ùþ›œ´Î?¸
o_v?ßñ4½™JŒ?¿V'ÌD3-?àe¡3Zº?¿V'ÌD3-MIXED4FGL J1808.4-3358?ïÚ;,HTÐÀæØnÁ~»À9…ëOnÓÀ;ÙJr'@pޚՃÖ@Íþu¼D¿?ÀN¢dïBî?éV؉™qV@#4h‡¨ÖM@ð™/¼[;?ïõÞs¾=¾?Èz Ûmé¿àEæÉÎË¿êøToÃÝ:¿ïÿ¥'(^?îK]@ÍЃUNASNone3FGL J1808.3-3357?Œè›…8*í?²•M#©?ïŒ]'´%•?²•M#©?ÀhýÍÿ/~?¼Â&€I?ëåÀŒ€4 ?¼Â&€I?Çs4L…6?°[g¯¼œ?ê?£2ìÞ²?°[g¯¼œ?¥˜Q×p•?•1>Ô`›Ê?î¦zâŽ÷?•1>Ô`›Ê?§5EÛL.'?Æ.O&aq=?¢/À7?Æ.O&aq=?›™ùµ3?£È‡°Èf4?ï#07;'¸?£È‡°Èf4?¬%WGCô?©üŸ§3½?î=®Ú§¡?©üŸ§3½?;Ô$eñ€?4%	@?ïü…{nO-?4%	@PSR4FGL J1808.4-4521¿ãûØ°¶8À'úƒBØÃÀ:>ýž%ðUÀ;ëø§F*‡@Öáü3í˜@á՚ѧþ?Í»{Ep¢?³š¾‡ºŸ?æ^æªÄdH?ÿ –˜³?³?¡6ÿ½Ý=*¿é†väÝ¿ã@+~³å¿à)¡N™Á¿ïúîéWG¿î?™UNASNone?ïîâ'9‡?w]…ÿ¢N×?aäEë¥?w]…ÿ¢N×?ïÔÚ©É~?ƒ̓¨'?u'« õ?ƒ̓¨'?ïZì-Û?ŒÍƒ†%×'?"¢}3€Œ¸?ŒÍƒ†%×'?ïԙq>d?]0œúOþw?u³t,"Ú?]0œúOþw?ïî^Œ=?cn'úZ ø?a¡sѳ?cn'úZ ø?ï^ǺO'Û?¥ìùâxx?"'°è:?¥ìùâxx?î¾w^}±(?™f6~Uì?¤ŠµQƒ?™f6~Uì?îÌs£2A?ŽþçÐT?£8ÅË$ ß?ŽþçÐTAGN4FGL J1808.4-3522?Ï$][¿ˆ/À•–\Î70À:ôj{žÜÏÀ<aÏ'ðà@@W¸"Ç?ú«»Š…) ?Òt¡ýì)‰?èÓ €étx@
†ݒî@g*÷O'I?ïù'áê@P¿íßRáNd?ÝÊ®›¤6¿æÄ}ÈØ¡¿ì•à<Z¿Ö×¹ºÌD<UNASNone3FGL J1808.4-3519?ïㄿöX??|—ñkm,m?l{?þ©?|—ñkm,m?ïw—iq;_? ú~ЄV?'
Êù\$? ú~ЄV?íoS•(p·? ±Ýto%˜?´…cXtHB? ±Ýto%˜?ï85ë86—?'÷ˆ€JÒ?˜ùBœhÉ?'÷ˆ€JÒ?ï/:¥9Ø5?¤:8"?š«QåÁ_?¤:8"?íÎ$!À?Âî/†^#?·YŽà¯·ü?Âî/†^#?äe½
P՟?»®ÙkÿØ?×4…ë^TÁ?»®ÙkÿØ?í°nåTÈ?¥MdüÅ=?²‡ùrÃ?¥MdüÅ=AGN4FGL J1808.5-3701¿î!hÁ›§wÀ \¥ß"9çÀ:%а‡éÀ<Ö¿•@raÆn@«ñ'l?Äær$àŠ?ÞÿÛlø§@'c/@ñÑHÝi}?難¥¦V¿´'¸N»yé¿âÁ' ÿT	¿çaÃ3ÆÖê¿êYè©¢%Y¿ïþÏ´ÙéUNASNone3FGL J1808.4-3703?æp¨,7-?ÉÛn®¼õ?Ó¯§'æ?ÉÛn®¼õ?åº6Á¡å1?ƱæJ)øU?ԋ'|¼5?ƱæJ)øU?æ'«âé¼?²qšA_Eá?Óñ°¨:,ˆ?²qšA_Eá?ꉃ辁?¢
4š0\?ÅÙð]û©?¢
4š0\?À×kÐøDd?Áþ¿OØýª?ëÊ%Áîç?Áþ¿OØýª?Á»QÈÖ?ÃéFݧ?ë¼Q+¹
Ë?ÃéFݧ?ÀLôÿŠ©?®èqkm°^?ëìÂÀUÀ?®èqkm°^?Í»d¯ÿ?­ƒÚa':Á?è»Ñ&ù"?­ƒÚa':ÁMIXED4FGL J1809.0-2853¿ë¤•µx66À­Š—ž×À:]xFÜ]À;އ$L£@v ís`@è«ÕÜ@?ÒíýÐ?梐MÀ}3@ÃèPïÝ@%&¹Óø?î)<7B·¿Ô€ûþh¦2¿à°ž~蝿æ¢CŒFÊÀ¿ïÿÿ)@k*?ìôí²öaòUNASNone?Û°9O'?ÑyiÐu›/?â'ãsØ>ñ?ÑyiÐu›/?ל«àv«a?ÎzÊzÑÇ!?ä1ªĪP?ÎzÊzÑÇ!?â ä¾Â.?²Ú_HW50?Ú¿Ì6'{£?²Ú_HW50?âO±éó?´U¯2RÑ?Ûa̜-ü?´U¯2RÑ?ÔôȩQØ?Òj˜Yþy?å…ͬW?Òj˜Yþy?¡,Ÿ;?²r…\w""?îîϽ(P<?²r…\w""?Ád
£#(?«uÈßüV2?ë¦þü—76?«uÈßüV2?°Áû=œš_?¡;7Ü·¼Ê?íçÀ˜ƒft?¡;7Ü·¼Ê	MIXED4FGL J1809.2-2726¿çMÖªœ ]ÀÞ9ܚ À9"©³`ëÀ;32¯È@ÕÜÔVÙÖ@w¶ :‹?ЛB;8æ&?Ê扷N``@
Y*f—@MŒ£ ?ïûÏ^¢wº¿ÙEíÊ»{¿è"d~.Ú¿ä-œ»	h¿ås°Á©X)¿ïÿýawUNASNone3FGL J1809.2-2725?éôš.?Ð…IwåŒ?È-—G¯Áú?Ð…IwåŒ?㊢Uä<?ËÏèˆóŒ³?Øê»U7ˆ?ËÏèˆóŒ³?ì•qo•s?¦"¡r€ûé?»TtƒWk?¦"¡r€ûé?ê‹U½»{°?¤î¢€5)	?ÅÒ©	>?¤î¢€5)	?èýÏx£Z?ÆÅP¿é˜?̹r—?ÆÅP¿é˜?»}×þülD?Ôª#Z£?ìE rw?Ôª#Z£?ãmŒ€´ùÐ?¶zŒ§üÖ?Ù$æþ–`?¶zŒ§üÖ?ÌF6ÇV/?³óà1ås?èîyòN*t?³óà1åsMIXED4FGL J1809.5-0816¿Ô·YÌ,Çg@¥ÊÞ¶]À9gÙÛ©¢À:ì™+µ@Ꮐ[@ôØý\·'?×T=ø´?âÙ`.@÷ñ"íjÒ?úe–w¦)Ë¿·ZŒhƒ¢?ß:…\ '¿êž`lQb¿ëÜÅ}Î¿æÈ|`x»©?ÈäD˜`_UNASNone?î"ë1ðE«?·œâkò?§±LÞgðM?·œâkò?Ó·1n{Íp?Ê׍%—ê?æ$gHÂH?Ê׍%—ê?èãyª	b?²'(ŒžÛä?ÌrW¿Úv?²'(ŒžÛä?ᅅP†?´ý傿ý?Üôõ_èóÊ?´ý傿ý?䁻Õ*G?Ò–›"ͧ?Öü‰øU«r?Ò–›"ͧ?œXnš× '?²zQ¢+†?ï<ŠäŽÏ?²zQ¢+†?àwUŒyu?¸PܼÆÿµ?ßTç
æ?¸PܼÆÿµ?žaþ«b´?Ž+fÌ,?ïð¿]?Ž+fÌ,MIXED4FGL J1809.8-2408c?ê×<$H‰²ÀDÍt'yÀ9$«Ô.ÁÀ:{Åyò4e@;€3ìì@>üå™Lm?Ñë>|è]ø?ã¤WB‡'@d>mùÙ?ýƒåîy¿ÛO[²Ù1¿à¾Ûrþ¿çŸTžè¸ç¿ëXÚϐ¿ïô…¾Eu€¿ïüø^KòUNASNone?¸Ö6vPR?ÂcXª8?ìå91=Ôf?ÂcXª8?»‡ÉÚÌa9?¿`'ô‡/?ìĦsÙ?¿`'ô‡/?á~´À*kÓ?´»ž"yè?Ý–«(Z?´»ž"yè?ÂI›6t'¼?¦¢
zt·Î?ëm™2bö?¦¢
zt·Î?³t¿ÙÏ^?¸Ü؎››?í'è Bô?¸Ü؎››?€Lèyó)?HIxw"?₩Ì24?HIxw"?Èæ9t.¿Ë?°¥.áàrV?éÆq¢ôP
?°¥.áàrV?fsQ+¤È?WöM®Bu×?ï錯è?WöM®Bu×8MIXED4FGL J1810.2-3054?âšÝ[1ÌMÀfù3]$žÀ:{ç¨ñ%rÀ<	0pá¬@g0{óÁX@D'¾‹Áj?Òٛ\'R(?ë¬<Ԝ¤ç@Ñ÷ÿ€~@@ŽFø7	?ï÷`‰­"L¿á1;A®A¿µù3¡ÜÍæ¿îÇ[¾í'¿¶",maZ¿ïÿѧ' ÖUNASNone?ëÉzTQ]?ÈÔ©ƒ$?Ù?äÚ®ºŠ?ÈÔ©ƒ$?Ù?è
Žüçó?Ë`ìÛFHu?ÏÉż`6?Ë`ìÛFHu?é,(h€?®JY°×"?ËO^]¿‰ÿ?®JY°×"?ëûì[?¬éᤂþ?ƒ´N"?¬éᤂþ?èwIØ2¨ì?ÎX"~¸ N?Î"؟5\P?ÎX"~¸ N?ÅF=.½5^?Ê"¶"2Ò?ê®p´P²©?Ê"¶"2Ò?ßiÿ¬·ÈH?»jž\:Ø?àK)¤Ü?»jž\:Ø?ÙÏï•éO©?ƗZ‡ˆä?ã5X+?ƗZ‡ˆäMIXED4FGL J1810.3+1332¿ï`_4ݜ@.A•övêÀ:eÜyhÀ<¤~Ïé¸@iÑãâèî@k;¸<òÐ?È÷èÔë?Éٕ2+Ì7?ÿ¡Ž«)?ù½X›L¢? Õ`¿â4Šˆ×¿âÚìJ@•ò¿æ¦]—ŠË ¿ì¬…dXo-¿ïÿø¨ó©°UNASNone?íþr£Ç¬?®ï¯¼xF?°<l™?®ï¯¼xF?é 5qžJP?Ä † 8?É*9†ÖÁ?Ä † 8?î2–°†6?›Æ7 A'Æ?¬Ö"øzC¡?›Æ7 A'Æ?ëBÓáؼ?ŸOVON.?ÂõÀ°x?ŸOVON.?ãTEX"ƒÅ?ÈÔ¬–Ô÷?ÙWuNØøw?ÈÔ¬–Ô÷?Ó¾UM´ò?ÍÁZ,5+ö?æ Õ{Ù%‡?ÍÁZ,5+ö?ç¢r—]er?·Û†nCªz?лÑE5?·Û†nCªz?ØϏכTQ?²'·Ó¤)?ã˜82U×?²'·Ó¤)MIXED4FGL J1810.4+1700?ïñî…ëM'@0ŽÓǒÑ(À:l0 ±»ÏÀ;ÇVpOu@™¾JÓãÂ@Þ?©c;?Ñ8š{@èþ?ÒþÄt¹@b¼ºh?ú[oó¯¿ï¢36ÌE?ç†tX—pÊ¿äÜþޗÐl¿éÌ«ßí;¿ï°ÿ笿ï^­À1ËUNASNone?ï8ÿcU˜k?¤.úó'Š?˜à"•$"?¤.úó'Š?æ+¬ÏùŸ?ÊàLF>?Ó©ú¦`Á?ÊàLF>?íx‰å­«? }ç\Q+ð?·;±@†+? }ç\Q+ð?麡ìEÛN?¦¶
ˆGÅc?ÉxNè'È?¦¶
ˆGÅc?çÃÎÌVZ?Ç1¼GÚ¦?ÑôxbgSK?Ç1¼GÚ¦?Ð3°±Ž,ÿ?Ðô¥¿?çæ'§8é?Ðô¥¿?㹤\rá?¹ä+àðy?،¶ßG=?¹ä+àðy?Ìpý–÷±[?´¯(~dº?èãÀšB©?´¯(~dºMIXED4FGL J1810.5-1415¿ïÎTgÇu±@·|ˆçš®À9(ê°£À:ˆ¿™Þb÷@ÕÒmrÊ@ìbÿ©˜ë?ÐÁ˜ÜZ^p?Íîryo,´?üQ*"ÿ&?ñ?ƒxšñ]?ïb´•žbV¿çWy-éGW¿ë:§0[Ÿ¿å+,Ôt`û¿ïÿü¿ÙŸC?ïÿÊjåQUNASNone?Ú, ©Ð•Ò?ÓBôqV"?â鯫µ?ÓBôqV"?×H쨩"?ЁŒ y?ä[‰ó««6?ЁŒ y?åª<ò¼ÿ?²—vhaõ0?Ô«‡Â†?²—vhaõ0?áí=¯|Ê?¸TÂkBÆ?Ü$儡m?¸TÂkBÆ?ÛZøýàÊ?Ґ#ý=ák?âR󃁛?Ґ#ý=ák?š¹cÔßÂ}?°ý¨	ÒoW?ï*4á",?°ý¨	ÒoW?ße2nè(?¹¡‰½ƒƒ®?àMfȋõl?¹¡‰½ƒƒ®? ŒÜŸb7V?"t´K»Y?î÷263Ú?"t´K»YMIXED4FGL J1810.8-3347?î'm¿²CÀVAb ßÀ:<piõg À;¾9ìN@ád^y]@|ªu‰ð?ςe"oä?Íöc7‡×@œd…D@³jÑ?¿¸v×LØuÍ?îx`äÇ?¿äxrØd°"¿á,|Ë,¹œ¿ãúÍ[h£¿ïü½Í«oUNASNone?ïóýْ¶"?ZDÝì6?XL}˜Z?ZDÝì6?éÒ?˜zÄÃî?¸–ê×i?˜zÄÃî?ïu‰Œ†5º?ˆ¨")	†?'NÎt`²Å?ˆ¨")	†?ïžÓ¯ü#?k¶dsÞ8?ˆK?@÷[?k¶dsÞ8?ïâ[ىb"?w¨Í¡+†Þ?m¤&Q´—?w¨Í¡+†Þ?í¢'Ì?Á}0'S×Ã?·2ër{ÞÎ?Á}0'S×Ã?ë®7‡?¬þݽ¡:í?ÁG!ã»·ã?¬þݽ¡:í?í-}Ä?¡·jˆª?¶—7ô]ìb?¡·jˆªAGN4FGL J1811.0-2725¿âSŠIM/Àh"!'÷¿À9ëˆêá‹À;ZÆü©3k@Þ´\"~Í@vœ©ïR3?Ïx´‡0¶V?;:bÒ]@rpŽ@*;±±éG?ïّG=V¿¦©aD¿¦SÛÓ¥Ú¿ëˆÎ™«¿ÖЀáf⸿äoTˆ'UNASNone?ï/,ÌDoN?®-lì.ÀF?šftz<?®-lì.ÀF?îW"Å8*?±â¾v~Ô ?ªÓ¯îY_?±â¾v~Ô ?íê0×›ˆ? 'jÌã¯#?°®yGç
Á? 'jÌã¯#?îyL¨áFh?åT6IN?¨k5s£gƒ?åT6IN?éxéãÞâ#?ħ¶t¾g?ÊXp"ws?ħ¶t¾g?ã…Â&" ?Ò~3?P+?Øô{³»¿ð?Ò~3?P+?æÃ>øXc?µxÆÍDÆø?ÒyƒæO:?µxÆÍDÆø?å5'mØö?½NšÂ¹x‡?Õ"û$N?½NšÂ¹x‡AGN4FGL J1811.7-1442¿íêE2º?þ	üD}ÞÀ9ÖÄÍ$À:ÿöÅĚÏ@ŽEµì¶w@Ã%Nn"?ÐýGþœ?Ùp ¤eP@è%@+i:?öcˆm¢Dä?ꐦv î?Àá®Ú÷³¿ÚڞÜúlm¿ä½ì)‰fF¿ì?韖]пïôÞcβUNASNone?ݦŠœ^ã?Ð9UJ6?á,º±þP?Ð9UJ6?Åé	 ¬w?Á&ß捛½?ꅺ=—Ôâ?Á&ß捛½?ä¸?rÂÑ]?´#cÝJ…?֏z]G?´#cÝJ…?ÝxÉ⯱?°¸–€|À…?áC›¨~(?°¸–€|À…?¾ÇXÕÀM?»D«'ÏÝ?ì=‡åGö?»D«'ÏÝ?ˆ.ðÕÖç?š!º{>…?ï‰ßDs¢d?š!º{>…?ÐõÎNé-g?»[Þ7®B?ç…؋iM?»[Þ7®B?­™
ßdõ?–Ûqk­A$?î&o!î3Ç?–Ûqk­A$MIXED4FGL J1811.9-2336?҅8eÄw`À¬|•|ÔgÀ9\Úx†ú[À:¡?´‰	@ð"댫u@e€éŸk?ӓI]ìð.?áK.g˜@Ê÷	·8ç@g|"¤b ¿ØÏ[†I¿Üw†´º‡P¿è7¾³.–¿ç©ÇÁJ¿ïÿûÎBÓ?ïCÿ3QfUNASNone?ÝxH'&Có?ϟtDJ‡¹?áCÛ¶ìÞ?ϟtDJ‡¹?×¾ü»¹?Ð"-a
Å?ä| ¢#x?Ð"-a
Å?äíæšÔ,=?³.[³$?Ö$2ÊW§‡?³.[³$?æ`Š`ãçé?¶/‰n¶éw?Ó>ë>80.?¶/‰n¶éw?Ô»‡nã|?ͦzp½
?åô"<HŽB?ͦzp½
?"—–ˆbҘ?©Ú-t·ŸÚ?ïcCK¯*û?©Ú-t·ŸÚ?Ëã#L¦?²11
Ôù?é7,ù–?²11
Ôù?©Ã4ÆÑÎ#? £™˜Z
ï?îc̳wf>? £™˜Z
ïMIXED4FGL J1812.2-0856¿®³xp‡°@ãâ"À9iÀv}4ßÀ;…nij'@I†¶º'@{©f–7?Ñ3a×5†?éU—¬Y¾@Ót62Áô?üq˜ç%á?ïðdìé¢Æ¿ÕUÕõjzÈ¿é®Æ¼èS;¿ïÿ–Aö¿è»À½Iø¿îQ9]ïŸ`UNASNone?ߖã•Ò?ѝw›S>R?à4Žµù?ѝw›S>R?¯ôGk°D?±SZ}Ìu?$ù¬?±SZ}Ìu?äà´ëQ»?µž4ÉÎO5?Ö>–)]؉?µž4ÉÎO5?¶9†¿\?ŸbPc7
m?í8Ï'×À?ŸbPc7
m?Ș"ž7?Í@ØÒ……?éÙÚþØ|r?Í@ØÒ……?}½r¶†²]?ŠÆلu?ïą†"?ŠÆلu?׳ß!?»PfŸÇ0?ä|÷>p?»PfŸÇ0?^ïºIr$?U?N«Óè©?ïðˆrn¡7?U?N«Óè©MIXED4FGL J1812.4+4441¿ï­3ğùý@9TgÓMðÀ;N'™ð×nÀ<Ž˜÷³*d@yòŽÖr@ ؽ›×a?ÇbY&D¿š+WÅ®K?Ó4ý¾1@ÊæÞpä¿å#ãŸw),¿Ý$	_$RÆ¿èr¦äÌÉ¿ÑÀWs"\¿è™\þØ<¿ÔðáxÚUNASNone?ïù'|'v?Lÿʀ°wv?I÷î4"p?Lÿʀ°wv?ïñœ˜ë?b˜êâ¶À?\ÇÒä'U.?b˜êâ¶À?ïßça¬ 
?sèÖ.$Ÿ?pOÍ?sèÖ.$Ÿ?ïö5Wêf?:U£…;™?S•P
6Á.?:U£…;™?ïàNù|?o
?Î?o±v%q
?o
?Î?ïÃM`õ§ü?'Ä4¿Ð?~YOŒ9æ?'Ä4¿Ð?ï±WUHÔ'?‡*`Ó^Ê?ƒª*¨û'\?‡*`Ó^Ê?︡?¼i¹?s,ª‰Õ!?×°6å¶?s,ª‰Õ!AGN4FGL J1812.8-3144?ìj¨>ðM'Àýœk1˜À:'È-*ÛvÀ<0æl±C@Ž!AÄ¢?þ_æðd'?Æz>ŠJc?à·l³‡i@þ•`Nõ1@')ó?ïÿæj,Ą¿ãšÀá?µ¿Äx@Ùd	ë¿ã,æ³'à¿í…·š5 Ì¿íؾópPUNASNone?ß*ômÙ*?ÒÕ)Š	{?àj…Éjý?ÒÕ)Š	{?֘Û
I§`?ÌÞ·vàmO?䳒zÛ,P?ÌÞ·vàmO?×ík
™?³þxó/-?ät‰xJz´?³þxó/-?Þ'VÙð;?°‡aKFß?àì9T"ã?°‡aKFß?Ñ|M:gÒD?ÎvUš·?çAÙbÌÞ?ÎvUš·?ªÌ¡»žs•?¶¡V<Ò¸,?îS5äŠÐö?¶¡V<Ò¸,?¿åç¡ Š`?ª!~ÉÂS?ìCËî´?ª!~ÉÂS?¸þÉXªå<?¤GÊ'è^?ìà&Ô³©™?¤GÊ'è^PSR4FGL J1813.1-1611¿´¸÷òò#¿?ë@dïmâÀ9.ð®SeÀ:J£Üºî@øÓ4ð͈@i:Áœíâ?ͳðÈT˜?ÀVT_þ˜L?õ-ŽxÔ'4?Ø٘,‡"¿ë³Na	y?ï2a|ÚQ¿æÙþäw
~¿äHîៗµ¿ë¨a}ÉY{¿ï¹úݬCUNASNone?âo	'ûÅ´?ÕzZná_+?Û!ìÚt™?ÕzZná_+?Å•_¼~?Ė*jH‹?꼸hà?Ė*jH‹?ãî0A2È?¶%C+ÜD?ÙÒ#Ÿ}šq?¶%C+ÜD?Ó5§¤|]?´•ØxÍRK?æe,1-ÁÒ?´•ØxÍRK?Ö³ӂëÐ?ÓJ6Œ{p[?ä¦s–>Š?ÓJ6Œ{p[?'î¯ø5V?©K·JšÞ?ïpŠ€]~?©K·JšÞ?áKs·‡Á?¹·fÝÑú?Ýióð~?¹·fÝÑú?'Øèû†?†ò]h"z?ïq8¿!œ?†ò]h"zMIXED4FGL J1813.2-1128?ì&E9£˜T@Ȑã²°À9.@q	W˜À:¡»á¸@‹Ò@MM@SÝͦ?ÆðtöL?Ò}PbÃï"@ÇÅ&^?éÒ°;¾ê?ïO+.?®¿á<W3Ã{ë¿æÉvÁ}cX¿æORîº]^¿ë€uf¿ï³Ñ¾¤UNASNone?ÍäæUg™?Ë^¸²Žˆ?è†üFj¦?Ë^¸²Žˆ?±‰/&#Ï??²Õãïªb?íÎÚrØ?²Õãïªb?âf&'²o?µB}¶H­Â?Û3³Öܛ!?µB}¶H­Â?»	³
³ó? Úõ†3É!?ìžß©žI'? Úõ†3É!?½ud}zv‹?Ê|PчOH?ìQSpP±/?Ê|PчOH?ëÊг‹?‹G³5¢*?ïÁâ(‡;Q?‹G³5¢*?É|Ä°ø¹?°8†Ž{¹?é ÎøSÁÒ?°8†Ž{¹?f+ç+t*P?W&éòw)K?ïéÔÄ¥?W&éòw)KMIXED4FGL J1813.5+2819?Ыˆ±ŒKö@41ÿ?àHÀ:Ý\úŽ§À<­½MÓÈj@Püi¤&?ûޑÖV¹J?ÌðÔ¾Þ¢?àM´ôhó	@jÝÄkÕ?ôÐÓÇè·d?îßÛgšC
¿ãç- I¡Š¿Á瘋§"¿Ü«´NPÅë¿êtÝAäüÄ¿æPazChUNASNone3FGL J1813.6+2820?⥐=­é?Ï+=ñR=:?ڴ߄¤-á?Ï+=ñR=:?ÖÅPŠ9³?Ȝº³?äñWºã'?Ȝº³?ç náùÉt?²œ_Þ}?Ñ¿"<m?²œ_Þ}?Þ¤Ìåö?°¦åÓñê?୙$ó?°¦åÓñê?ӸЂ:¿?ǖóC{w<?æ#—¾ðb¡?ǖóC{w<?¯þÏ´uÍh?²Aê'Eò"?îáÞy?²Aê'Eò"?ÓG³æÕj3?¶F¯fà_?æ\&•Jç?¶F¯fà_?¹$ª¯@ŸØ?¤r{ø'Ü
?ìÛjªì?¤r{ø'Ü
MIXED4FGL J1813.7-1152?æã"î^íÌ@IÅÓï×À8—¡Vý<×À:I">¿@0êp ÏX@3¾sm¶?ÆZ"Zî
9?ÆkúdŠ™!@D,Ý®œ`?ø9€=Òô¿ë@tdUë?ï^µÍ¬Æ¿åßÁ œ,Ç¿è½^®(¿æ˜~±¶ÆÑ¿ï÷ýO0ÀUNASNone3FGL J1813.6-1148?ãøúƒP?Ò©0N–*?Ø
ùÇñ`?Ò©0N–*?Ì_Ÿá®?Ç»)ُ >?èè¼?"?Ç»)ُ >?ާԚÌt?¹õÞ:Ä?ଲ™Å¹?¹õÞ:Ä?Ú%æŸí×Æ?¶Ü†®Vž?âí°	?¶Ü†®Vž?Ɏõ—­lp?Ç®óþ"ðè?éœBš¤ä?Ç®óþ"ðè?žîµEjÄú?±Ðh&0ˍ?ïŠUâhH?±Ðh&0ˍ?א™Î®à?¾³ê'?ä7þ3¨?¾³ê'?›îŠ²'?'d':z†K?ï ‹ª‡l_?'d':z†KMIXED4FGL J1813.7-6846?ÙT5SkYbÀ5Üك"t—À:ÂÀ<G³"ÛÈ@ȪWVþê@çLû‹&?Á.,¹•?ÉvÙ%J½>@]o¿«|@æW¢Ô*å?ï'È#ð ¿à€Õú¿ßìÐÃ|l¿æÜN_‰}m¿ë&ojñæb¿ïÿö$´ë/UNASNone3FGL J1813.6-6845?îÿ'XN9Ž?ŸYéQÿp? Úyd™'?ŸYéQÿp?ïz¨â9?'©¨·B¾?ªÿ|à@ì?'©¨·B¾?î…á‰zñ?™¹¾.!Ç?§¡çdk­?™¹¾.!Ç?î•?ªpª?‡"ÊódÙL?¦¬]á'e?‡"ÊódÙL?åK·¥¨?ÅC<ð?Õh´åò°?ÅC<ð?íž>}ze]?·	uëD?³¼?·	uëD?愡n
…Ñ?µkV±¯¾^?Òö½#êô^?µkV±¯¾^?çÕ÷¦$d?¯…Û·àÒ?ÐTö³·8?¯…Û·àÒAGN4FGL J1814.2-1012?ç™÷_>÷.@ÑăR/xÀ9u]ù°Z¦À;§ž?È@†ò¯	˜Z@$Øý\·'?ÓãҢϣA?ïÎÿ!]ȳ@v9þ(k?ÿü¢¯»Å?í½Aߞ`©?·ÔÂ]³¿íw6,â·¿å³:Š?‰ƒ¿æ4á‰t¿ïÿèîkƒUNASNone?×O"@á`q?Ð÷ëtÚv?äXnߏOÇ?Ð÷ëtÚv?Â9QI7›<?À~"LL×?ëq«­²1?À~"LL×?æ¶9I;¢?³pã͚R&?ғmˆ»ó?³pã͚R&?Ïô•yà|é?²òޔ¬g*?èÚ¡‡àÆ?²òޔ¬g*?ÊnúZ_Ù?Ê7pBT±?édAih	»?Ê7pBT±?ˆÀ£œ†?˜>@o–AÊ?ïœÿ•ªN?˜>@o–AÊ?Þ$Ý´?|?º-c>Øqµ?àí'%àAý?º-c>Øqµ?‹™(š"âu?€;w…¶£?]`z¶?€;w…¶£MIXED4FGL J1814.2-3000¿áÌ
õÒT¡ÀΡáf·ÅÀ:ØC1­÷õÀ<mCÖïe~@0ÒĚ?ü}s]Å­õ?Ô»´4çh?瘒üÕ©@;YÎy@TÀœ<â	?ïýî½ãOñ¿èø¥˜«]¿Ó/ÕÜ¿çpi§Šô¿çg'…€Þ¿ïÉƽ¿ÐUNASNone?ïæ–Íar?¼±IÆiþ™?ŸC--3	°?¼±IÆiþ™?ì5v"kµ?Àz3J¸¾?¿NTKÜ¢X?Àz3J¸¾?íqEý²•?¡¶æ"◵?´tÎZY?¡¶æ"◵?ì&z%"•ý? 'æWp%î?¾Ì.ÓcP? 'æWp%î?ïm5èý?£ƒ÷¹^?'Y\"üÀl?£ƒ÷¹^?Ùä-ŽPË?҅ùæØ´?ã
é8×ü›?҅ùæØ´?êG
W?±/õDÄ?Æá¿Ëåú¤?±/õDÄ?ã0¹žá?¼«•?Ù۟ЌÂ=?¼«•MIXED4FGL J1814.4+2429?ÓTW=²Í@22ç³ØàÀ:vÉ5h—™À<‰a=2@'ìðٜi@Yã¡$¨?Ø1#ùÚL?Ó´B|Ò8œ?ÿàç6Ÿ?óDCƒãNï?åÉl|«¿ã¤­><%Ë¿é²¾=èÃοåq؊p0ë¿é+·sŸ4
¿ïÿÈ!ÂGŽUNASNone?ì>2BûÛ·?Ƽp˜2U,?¾mè!"K?Ƽp˜2U,?ãåUµG°?ÍØ­‰C>?Ø5T•ÙpŸ?ÍØ­‰C>?í9"&œ?£d(f¯3?¶7Ví]#?£d(f¯3?èTõ™?­®±.]?Ïî¬+Ó©œ?­®±.]?ç€zܕÓ?Ít1™ïÅ?Ðÿ
FÕÒZ?Ít1™ïÅ?¼?Ns?™¤d?ì|8V1?™¤d?äÉ$¦(¸?¾´%È!Ó?Öm·Ð³®?¾´%È!Ó?¿»ìÈÉ:¥?¨|cèW£È?ì'fæØ«?¨|cèW£ÈMIXED4FGL J1814.6-3621¿¬U?ÎQP7À!ëÒRGËqÀ:±šW.ºþÀ<,3øUÔ@dn¾Ï‰?ýAŽXø?ÒKÝcß$?Þ¼Øc@§"©GŒ‡?þ<sÿP³?îö+jçÕg?ï†G½Xæv¿×(èÁõÙ6¿Ë1··¿êJë€ìúj¿ïõXÝç¯UNASNone?ï©øÉ¢BW?µNöq¶C?…ÍžN¢4?µNöq¶C?î–Ôå—k?²Š¹ñ)­¶?¯–'®6íO?²Š¹ñ)­¶?îsuI€w?–d‡q¬sD?¨È«j|uœ?–d‡q¬sD?în‡Ð¡÷?'ÔE¯:)l?¯É>'?'ÔE¯:)l?ï‰ ÐÇû?'wn">ª?·øR­9?'wn">ª?çúF!nÜú?ÍYX©íØ>?Ðs½"F?ÍYX©íØ>?êèI»"r?®GZÙ%±Ò?Ä^Ù²7©?®GZÙ%±Ò?èXµ"€?´¨,Ä€á?Ν+ݱÿõ?´¨,Ä€áAGN4FGL J1814.6-2537?ïdˆ=HØÀ°LÎå«ÁÀ:qó·ó ôÀ;±rGE8ï@Ï0֌"#@x~…A?ÛÉ{"P?æãèb)•Ñ@ãÈ\$Ä@ÿ[g¯¼œ?ì'1ÆK©L¿Ê™ú<œ"t¿Õyëñ@¿çýB`wº¿ïÿþˆ0»Š?ïÿ£ÿywUNASNone?Ó=_÷·\"?Îú@tPV?æaP$Qï?Îú@tPV?ç@›wë?̦zeŠ?ÑÒÉ)Ä?̦zeŠ?åzx©ßâÔ?²â_a •?Õ¬@:X?²â_a •?ê藱7?¨\íÿ"?Ä]¡;#—Š?¨\íÿ"?Àø"*}Ø?È©z7S©?ëÁÚù5`Š?È©z7S©?»âF5b?Å_r£­ç?샷9_®?Å_r£­ç?͔iÏ&™G?´»²#ºU?èšåŒ6Y®?´»²#ºU?ÒÚïÓj©J?ºá
ßÔM?撈J«[?ºá
ßÔMMIXED4FGL J1814.7-3420?ïVöҍ^«À uæ6*^À:xv3cÀ;Ñ[§Æƒ@®Qäy;Ö@ëE®_ú<?ÑgC:è3[?ÞcK©Í@.ã,?öVwî¤
?ïã&@©?Ô1½|Í°ø¿áÜ4-n¿ç<¢³Ï¿í}Sþ.ïÑržƒ
fUNASNone?ã÷{FÈ;n?ΝïWaÍ?Ø	ro‰%?ΝïWaÍ?Í[7&ex?ÇtÛ¸ç¬f?è©26f¡þ?ÇtÛ¸ç¬f?ÞÊ
ä€Ñ?²›¹·ú¶H?àšúô
¿—?²›¹·ú¶H?À¨ŽÔï†
?¡Ü‹h Ê³?ëÕÜJÄ}?¡Ü‹h Ê³?ÐåÝ'k‡k?ÑÖl‡¬v?çlJ<J?ÑÖl‡¬v?¨êы©3?´ó§;Ÿ'?îqRçiÂM?´ó§;Ÿ'?Ásÿ<qÜw?°ƒ»éC?ë£0ãˆâ?°ƒ»éC?jJÌ0âwa?X‹w9ÁÆu?ïåµ4w ?X‹w9ÁÆuMIXED4FGL J1815.1+5917?î¸!Qg@;Ÿû¹IbÀ:áZˆâ'1À<D|	f@×lu:(@¿\¢˜F?Ðb\ªŒ0?æ­z¹Â@ê±ý=­à@áð˜XüÆ?ík9i®ƒ¿ÒîÍþ¾a¿è̀†£пêòI^ãL¿ð?ïÿ±%§YvUNASNone3FGL J1815.1+5919?âÕ8¯Û
¹?зB
Ž?ÚUŽ Iê?зB
Ž?èÖ-q?Éo÷ý…°?͋ü§IÊ=?Éo÷ý…°?è.ŽmbüF?°Œ&8íÀ	?ÏEÆJtè?°Œ&8íÀ	?ê{ë5˜"4?ª‹¹åè?ÆS)³/?ª‹¹åè?ÖCu£Î¯Y?Ϫ""`
?äÞE.¨T?Ϫ""`
?¹¤›Å?²#úÂ9²?ëQº–Ù¾?²#úÂ9²?Û©ƒ'ØE?·î'°3s|?â+>6"Ý9?·î'°3s|?Ê Ob¶%
?¶ÍÌW¤/?éWì'Rv½?¶ÍÌW¤/MIXED4FGL J1815.3-1336¿àyòAìÆ?ùæŠÁXÀ:µc#»ÇÀ;­iiP%²@h½}¤p@/%¿­*?Ն¼RV9?ï‹'!­@ØÜ@Þ¡@Ѻü•½A¿äúœl²±¿îd%ÿn	É?ÆÔ¨Ž¿äJæ
²û¿ïÿ¾[ðÁŸ?àRâ¥üÿUNASNone?ޚ¼
%Ç)?ÏùôŒ&Ñ?ಡùml?ÏùôŒ&Ñ?àdw¬h?ÐmŽ¼yv?ßÇÃ7§1?ÐmŽ¼yv?äF¯«˜Žq?³SɎéb;?×r ¨Îã?³SɎéb;?ã²#ýúÛî?¸ï3›Ï.?؛¸
H%?¸ï3›Ï.?É@³Ú¦W?ÍÕÌ-s3?é¯Ó	|Öj?ÍÕÌ-s3?«*[‡†?ºC»×6¦?îMZG¸ë?ºC»×6¦?͵yXj˜?´n^8:?蒡©ø%Z?´n^8:?¼ÿ t)G¢?®ZȒDU?ì`ñz×?®ZȒDUMIXED4FGL J1815.8-1416¿ì¾YÂi?ó2±-4À8¯Ö»cýÀ:<òô~Â~@ûèɂ•q@#¼ª ?Â-«3õÐÒ?͍eä@ûdg?ìiZ"›õ¿Ôû¿¾òCª?ëÄQh¨`¿æ9œf¿æ"‰!Q^l¿ïeDþ6ҿ撝'uÞ©UNASNone?ÕÚ¶¹~Ö?Ԅ†Ò… ?夣@"ù?Ԅ†Ò… ?±)ŽK9ì?´@j!¡?íÚÎ6ss?´@j!¡?ÙHþù'?·ñí°>™?ã[€ƒ6ðq?·ñí°>™?¶Õ`'ߢO?šóf£µ{?í%Sû;v?šóf£µ{?ÀÒ	Wl£l?ϱ7OÍrº?ëË}ª$×%?ϱ7OÍrº?y²@M…Áa?†¹V'áy?ï̛€q]?†¹V'áy?ÁCÛ!#f7?­u°p€?ë¯	7·&r?­u°p€?bhÛeà½A?Tv/ª€²?ïí—$Ê9Ê?Tv/ª€²PSR4FGL J1816.1-3908¿äûèÎWˆÊÀ$ù³ÃçÀ:Q¤nß±¬À;ðbMÒñª@P‰áÿº@
vÙ{0ù?ÌÂ*7‰?ÐGýûCÝ?ýVÝA‰?ò¨"pÃ6¡?ïýê|
<š¿åÁ`>¯¿åáù£Åm¿é=b.$¿çû¾Aě{¿ïñÁ—ådUNASNone?ïºû\¾X&?¬=R?ï­m?A(Æ"ˆ?¬=R?ï­m?ìÕãÁŽ‰?½GèÑ)¾?¹W á…˜:?½GèÑ)¾?îM•è'®¡?Ÿ"áص?«&¡yhÊå?Ÿ"áص?íóӊ½Cÿ?'àÓéq–?°acªñÇ?'àÓéq–?ïÍu}yÜ?‡7:MŸà?yEx¹?‡7:MŸà?ÛÔ ýLW®?ў"ûW¤­?⯁YÔ)?ў"ûW¤­?êœÛ4ˆN?°e²Bz&v?Ō"/áÞÇ?°e²Bz&v?àKÜö¡Ã›?¼œÀE¼?ßhF¼xÊ?¼œÀE¼MIXED4FGL J1816.3-2903¿ïæó£•	×À"ͅYÀ:"Ü·%››À<opŸM8@*ÓÄ[d@DEª.<?Òäç`Kð?ïÿûÎBÓ@Èd©ÍÄ?þr¥;¹>¦?ï'v1µ"²¿ãýô·ø¿Ò™#"™Þ¿ïÿâ£Î¦Â?ï؊p0ꄿïÿüoQÇsUNASNone?ß½`ÆòËÃ?Ô.€ß}?à!Oœ†š?Ô.€ß}?âÖ6&œeÁ?Ô=yšm Œ?ÚS"²Ç4?Ô=yšm Œ?ⲩô8T8?´AtƼˆ?ښ¬W?´AtƼˆ?íµ/"h›Ü?¬ŒZæ²Oi?²V†îrï?¬ŒZæ²Oi?àMiÆ©Xe?Ô晻íd?ße,r­O7?Ô晻íd?´
Fh"?ÄÝâV»'?í~~½,­?ÄÝâV»'?ÙèkFӁ¥?¼¸§*?³c?ãÊ\–?-?¼¸§*?³c?Û«iÊ7àÜ?ҚÏ*A"?â*Kä'?ҚÏ*A"MIXED4FGL J1816.4-0057¿ïC‹j¬Ç@_¾vÈ´9À:.Hè§À;_WƐr©@ïxŒÙ—¶@ˆ¹º¡Q?Ìzº0gý?Àÿìý)·?ö©Ä¿¸T@WKÐ
!?ÜA œ,ÆÝ¿æރ¾ôÚ¿æ¢:Að:e¿ãøèI*}¿ïüŽ[wõÛ?›^L€PJUNASNone?ïÌÒÏx×5?y¯_©ˆÏó?y–˜%WÕ¸?y¯_©ˆÏó?ï	85Ú
+?¤X´å	
"?žØùCì­?¤X´å	
"?ïÎê‰KC?'ænea¤M?ž"¦?'³?'ænea¤M?ïYÍIV?v‰
ù(Ûv?"Æ_ŸE?v‰
ù(Ûv?íët.C?¬ÊDfÖn?°¤_WiÎo?¬ÊDfÖn?ègaÛ^­?Ë%®[±?Ϟbx'…K?Ë%®[±?ëWê͔?²[ö·Ÿ›?Ãûš Tɱ?²[ö·Ÿ›?ê
F™0Vú?­LE±m©Y?ÇÊå›>¤?­LE±m©YAGN4FGL J1816.4-2727¿°ŸÁ
Y!Àªä>šÀ:EžG~CÓÀ;ÕbþÒÙV@týۅ¢@58[' N?Í$ɍþ?à†ü©3j'@µÇ`c?ü÷Ǫfp?ïœQքܿá÷ ¦éŽ¿ãƒ>
É¿ÜÔ»%_¿ï
•µŠé¿ïÿÍ'ý UNASNone3FGL J1816.2-2726?Çv"[0?ÆrÆâä!Ž?ê"` 7i4?ÆrÆâä!Ž?ÈÙ<'ùU?ÅÊ)€E8?éûI°ßA«?ÅÊ)€E8?Þ㴷χ	?³ûÖTÔÑP?àŽ%¤<|?³ûÖTÔÑP?Ò¢´Ø0Ðz?°2éƒF-ý?殥"ç—Ã?°2éƒF-ý?«Y#tÞ«?·7s_R‰?îJmȖ˜o?·7s_R‰?šuo
–ûá?ªÐGK?ï,T‡ÊAá?ªÐGK?ÀC雱ï?ª1NšÓ¹?ëï™"9?ª1NšÓ¹?"S&R+T?Ãèã†à?ïefÍ¥ õ?Ãèã†àPSR4FGL J1816.4-6405¿ë'A‰jÕêÀ4ŒfçÀ:V#ßÙÀ<FÒä>@$þØ;–@›¸€®?ÀÇÐy)·‰?Ö°Þ$
%'@÷jøœ^p@eÍ=`Ó?ïÞâ¾ÑŒz¿ÜTµ"0ѯ¿à€ÎۚƿåÖ½•!e¿ïüK_ÏÉV¿ï'nÂ6ïUNASNone3FGL J1816.0-6407?á%9d>ˆ?ʆBÿã?Ý˵7'ñ?ʆBÿã?ìæNøÁü?·>¶®"?¸Í§ã¡?·>¶®"?äGAå?µ«ôrÕ á?×p"²‡|6?µ«ôrÕ á?íh	8M?'¨d$Ò#L?´¿´ó½y?'¨d$Ò#L?»ÑSÍ»í?¸ÆªÂu€Â?ì…Õ†HÂ?¸ÆªÂu€Â?ß$ÅÙàÓâ?ЕeCÿy?àm–?ЕeCÿy?¾0=yL
?­"ΤUnÎ?ì9øPÖ~Ÿ?­"ΤUnÎ?ßí½È¢ñ‡?±@™Øk­?à	!®‡<?±@™Øk­MIXED4FGL J1816.5-1208c?èœ"e@Š	¾Å£
À9>'lVjpÀ:¡¨žð@þÓ xñX@!Äüó0?ÌòÇÞ%²?ËáÌ8RVå?ú€yK!@»t_οïòbüO?îþýÁ·Dû¿çIðäÚ	Ì¿áÇr_Ãßé¿ì|vÕIs¿×8\OUNASNone?éƽîQp¥?Æ;òŽA:¢?ÈåFº=m?Æ;òŽA:¢?é¿$ý6?Æ)ƒQX¸(?Él
'ì?Æ)ƒQX¸(?çbvõ!L"?²àŸÍÇ:ë?Ñ;½g»?²àŸÍÇ:ë?ìŊB†Ý?¡=pÍîA?¹Ó­ëÏá?¡=pÍîA?Õ6&]ô«?Éåfq–Š?ådìÑz«?Éåfq–Š?ÖÛf—}yl?ÓQùu*9?ä'L´ACJ?ÓQùu*9?Ú=¼'Ü«?¹²Á¼Vµ?âÀa!¶'«?¹²Á¼Vµ?×à`ß$#‡?Á­[OBD?äϐmî=?Á­[OBD MIXED4FGL J1816.7+1749?Ë>ùåߘV@/M߆ã´À:GI¡À< SúSÕ@@ƒÊû;u@XTŠ›ÏÕ?ðHÔÛd?Ðv	ý.êN@OÈ‹ñ:@¬ß¡GŽ¿â-ŸàÛwŠ¿ÝAÛ¢R¥¿¿ãßKà(IJ¿ÕÎN­=%¿î«A—z©¿ïáØݧ:—UNASNone?ë)&òށ?¾84ØWx?Ã[d4‡ñü?¾84ØWx?éq'´™ü?ÆfìþÆo?Ê9µ/™˜?ÆfìþÆo?í"+=ü?£y¬oXT4?·S^¦p#?£y¬oXT4?í(5k-?"[!ü¹€h?¶¿þUðrO?"[!ü¹€h?ÞyÝþÀ)?É´÷}jÛ?àÃûŸë?É´÷}jÛ?Õ4"™#ÊW?ÐxŒZÒñ?åe½³nÕ?ÐxŒZÒñ?âÄò³fI`?¹¢ì"šÉ?Úv™3m@?¹¢ì"šÉ?à[1P?¹›b ÍÚ-?ßIŝûË_?¹›b ÍÚ-MIXED4FGL J1816.8-2800¿ßéˆåcOÀq´xB1À:fVߋÀ<
çbzH›@ë\ђ.@ý'$ZR\?Ô¹A?:}?ï¬Zœ-Ȑ@ &5?þOL'S$¿Ç"(GÔ?î¼ZYê
¿çoÚ]ÙúÞ¿ïӃüº{?êÿ}úâ~¿ïÿ:Þ"_¦UNASNone?çpq¨eº?ÏTÙ~¿=?Ñò¯4‹?ÏTÙ~¿=?åK'á"Z?Òh© 9J?ÕhÜ<×K×?Òh© 9J?èþ2×)i?®ðïSÐÛ§?Ì4£[ö\?®ðïSÐÛ§?îH'qK>?¥€à~õ^?«v߸ëL?¥€à~õ^?áœõ'E$‰?ÒÞ'ýcÝ9?ÜƱu¶ï?ÒÞ'ýcÝ9?ºO4›"÷?Æè<Žj€@?ì¶lœá?Æè<Žj€@?Þ"_½L?½aÎÀܘ?àîÐws¡Z?½aÎÀܘ?ÞMÂŽå?Ñ¡ÿˆz§?àÙú82?Ñ¡ÿˆz§MIXED4FGL J1817.2-3035¿×‹xÉëF
Àœ…×EÀ9oßq?RÀ;¸ò–Šñ@Øä|û@؛7(‹?¶¢bk/å?¯Åäü"Ì?ö-$[)'@²¹c
–l¿ÞBkØ?ïÿɯæ¿æ-'?2D÷¿â§Òw0¹¿ä³!96¿á'‡N={UNASNone3FGL J1817.3-3033?ïõÒÐ¦?d—Ý
>h¸?TZ_¦êt,?d—Ý
>h¸?ï¡ðô'g?"ì‰êÙ$?‡ƒÃ‹º5?"ì‰êÙ$?ïˆæ[ǯŠ?Œ~¤J̓¬?Æhüæ?Œ~¤J̓¬?ï|$v'?v\æ‰úÜ?{}q<O´?v\æ‰úÜ?ï͖Käãx?~¶ü\ۘÛ?y4Ú]¸0?~¶ü\ۘÛ?췜×ð?Áçþ‡§K?ºC@X?Áçþ‡§K?îâPÜÞµ$?›~Ò<$'å?¡Úò4¨b¼?›~Ò<$'å?íh…ý‰È?£"D¶Xæ"?´»×бÁ?£"D¶Xæ"AGN4FGL J1817.5-1034?åþúÅ¿£€@³	ý¯Ã¨À:ÇíiûFÀ;Ù€9vC@©Š(b@ñ]¥Í"ƒ?ÒáO¦0€Ñ?ç»ÿTßUf@‡0[žŽ?ö7–§¡Å?çèQBgك¿²ªËÁµ¿Ö§e47?1¿ìm² {¶¿ïÿþó…õ?︣µ|N/UNASNone?Ø\$wÈRY?ѼvM¤?ãÑíÄÖÔ?ѼvM¤?¼N–w6~}?º¸ª–l£?ìv-100?º¸ª–l£?ã_…n"]E?²®JÛLj²?Ù@õ"×Ew?²®JÛLj²?ÉSýûe]õ?«L™Ô°yŽ?髁&¨ƒ?«L™Ô°yŽ?Àe=Lø½R?É6ê'?ëæ°¬ÁЬ?É6ê'?€£ÓÑó+?ŒÖü¤=x?ï½p°¹",?ŒÖü¤=x?À'ÏŽPÃÅ?­CyÿÚÈ?ëÛLkÏ?­CyÿÚÈ?"^ˆ¬Ðn?s2
OÍe?ï¹®…ö	î?s2
OÍeMIXED4FGL J1817.6-3251¿ÎÈd¤*¨[Àžm=ðüWÀ:Ò7yêÀ<€Èþ3:@hÆøL'e@ÛÈ:–ÔÃ?Ö¬]᲍?ïô×x!yÍ@'ƒ'à@_VlHS¿ïöë¹÷Ýó?ïÿÄ;-Óx¿Áí@	Û¿íO9ßÞè¿ïÖ´!…5ß¿ëœm‰pVªUNASNone?êE°™˜öd?ÈŠ9îýé?Æé=™œ&o?ÈŠ9îýé?܊饆É?ͅÍ>· Á?áºþ‹-<œ?ͅÍ>· Á?ãf[%‰f?²zºŽ	W=?Ù3Iµøí4?²zºŽ	W=?Û¹fNÏ­?´-ë2#?âu#Lؘ)?´-ë2#?äZ¶Înô'?Õ@‰Zå²U?×J'c"ß?Õ@‰Zå²U?¶Ž'ãù¬W?ÁÓªrÀù?í.-ÃeM•?ÁÓªrÀù?ÎóáՃ»È?³>´¡ñ?èCŠŸ?³>´¡ñ?¦·ýÙpZl?•‰}ïNiá?"­²‰?•‰}ïNiáMIXED4FGL J1817.7-2517?íHTyóÀª0À'+çÀ:–kÅJøÀ;¾}ík¨Æ@‰+Îdý[@º"¦6?Ö<€"Þ?àþ!†ù"@
X¥ÛÇ;"@‹4ԝü€?ïç¥*ÇSç¿ãe•®×ï¿á˜aÁ;¿åzJIˆà¿ïÿÿ" 5•?ïúµK¦ÇUNASNone?ãæ…/»k?Ñ<¥ºd?Ø3æõ ‰+?Ñ<¥ºd?ç*b ¨ä?Ì×PáfY?ÑÅ«;¾®7?Ì×PáfY?諶«çé£?±ùÜ."?ÍQ%P`Yv?±ùÜ."?ë¹ÇÁ—†ç?¥Õ-GВï?Áàù¡äc?¥Õ-GВï?ր?à¥?Ñfšyú~?ä¿àþ-v?Ñfšyú~?¹9¯‡Ä9h?áŞ@ƒ?ìØÊ>r"?áŞ@ƒ?Ú°¿½R?Ãà•Æ?-×?âô§ ~¡W?Ãà•Æ?-×?Ò¢²z™­?»Ì¡È€ü"?æö.¦Â³*?»Ì¡È€ü"MIXED4FGL J1817.9-3334?×bZ]n›À 'ҝÇ%ÄÀ:Ø"r8À<(ÐV©Z@RȲ5ò«@–¦ Z?¸m]ôþ?á¸W=Ôw@ 7 þ}I?þÀd*
ñ?ïþÎ!`¢Ø?ÀÄ,[Ø¿ÝÿFÃ*¿äu/dÊ¿ð?ïíßlÁÕUNASNone?·1ÿë'îÁ?Ån¬VÆÇ`?íÀdh?Ån¬VÆÇ`?ј~u•%?È\‡ÈêG»?ç3ÀÅ51n?È\‡ÈêG»?Ѐéöd†ù?²"õlöoÖ?翋ͼƒ?²"õlöoÖ?ÖªŠ$(?·Šö8
?äžøªºíì?·Šö8
?µSàÆI"?ǵ_ÂÍ?íUƒçDŒ?ǵ_ÂÍ?¦}iñ·ó	?±°á¡î?î˜)`»E€?±°á¡î?¹TOÓöä?®Y­yÙ'?ìßu÷´?®Y­yÙ'?Œßz¡¿¬?¨ð¿eD?Øõá?¨ð¿eDPSR4FGL J1817.9-1135?ï÷g!4Å@+àXšËÉÀ9H¬A<
À:ºŒã¨±e@]ÆYÁ@ßú¦ú«?Õ4<Ëbj?à÷–oB­ú@
ŒWâ?$Ù@¦o¾(ð¿Ö#IüMmò¿Þz"@Ÿ¿äkŒ–|¿ê¹ÂÅâοèkœ0LÏ¿ïÿú¡œGtUNASNone?çf¹&ʧ?Ë*äÉÝrü?Ñ2²kÞ²?Ë*äÉÝrü?Ð=X]¶ñ?Èu•zÈjŠ?çáSÑ}$ˆ?Èu•zÈjŠ?æ1oFP?³Ë²§çÍö?ӝ!×sÍ`?³Ë²§çÍö?ä#ŸÐÇ?¶Ä]ˆ-?׸ÀÄ^qÙ?¶Ä]ˆ-?Ø·Vå%Dn?ÍrCÎOȄ?ã¤Tm]É?ÍrCÎOȄ?"ŽeÏa?£Fç +¼Ä?ïg[ƒU×Å?£Fç +¼Ä?Ú<¸n_É?¸§wÖ¢ÏÓ?âáø£ÈÐ?¸§wÖ¢ÏÓ?¨@šeK¨-?œdvãf`??î{öYtK½?œdvãf`?MIXED4FGL J1818.0-1339c¿Ñ8ӎ»wÃ?ðWš5 Ë½À9?Ùx¬ºÀ:ZaՈ@­>'
@¸©õ1?ΟH/Cºj?ØZí!*È@‡#uP@î›×6ˆ'¿ïæ†|†c\?ïú^À՝¬¿à³%³A¿æ
ŽÏ;<¿í<ÜÊpÑú¿ïì¼Á¼ÎRUNASNone?Õ'ÓÉã†?ÒN¾º…Ú?år·=?ÒN¾º…Ú?Óá…|½Q?Ëœ¸F?æ=A¡Wu?Ëœ¸F?ßWÒò">;?µ@´…k*?àT†îàã?µ@´…k*?æàÊÁ(?±Ab›IªÀ?Ò>kè}ϱ?±Ab›IªÀ?ª")m6º&?²[:É£|?îV½i,"^?²[:É£|?¢œ'(ƒm8?°o? K[ë?îÖ6í@Ïm?°o? K[ë?Æw‰¹ãÍ?²r=•¼ß'?êb8'‡
?²r=•¼ß'?ÁyÚÌê©×?±®Ž«¸?롉LÅUŠ?±®Ž«¸ MIXED4FGL J1818.1-2000?ٟ`ôÈ¥‡À	 bvÞÀ9æk¤"ÈŸÀ;Æ¡Ú°»@)²~AúK?ÿ)¢üê³?ËæáK	Î?âÕm…>˜Â@)4AP,h@ŸJ(Åò?äT´W‹P¿è4%CâX¿Ês4j•Ë¿ÓìöÖBL¿í#¼Sƒ¿ïÿ·`)
UNASNone?֖)ì§Ly?ÉúeãšÖ?ä´ë	¬YÃ?ÉúeãšÖ?×Úí´…?Ë)ìûó{?äð‰%¿=?Ë)ìûó{?â2Å­§K?µŽ¬ˆb#\?Ûùšt¤±j?µŽ¬ˆb#\?ã˜ç©-G?°,¾Àh½?ÙöÎ0­¥s?°,¾Àh½?ºvðæ÷4C?¸§¶‹xÈ?ì±!ã!x?¸§¶‹xÈ?¨-q(;|f?µÛù.e0?î}(튪?µÛù.e0?Ï^Ü,CÞZ?¶Ë>÷÷?è(Hôïj?¶Ë>÷÷?Ä'¨2-3?¬ÊЫü)?êöó~´³?¬ÊЫü)MIXED4FGL J1818.3-1233?å+UÎ釙?÷Û¼Ú'.À9'0¤ãy·À:¶]këáe@ G9Oó@ݙÙZyÉ?ÊüÑâ¶C?´Æjˆ	#j?îXþý–ï?û´¦xz:¿ïç܈+³?ëÍ$ Ҕ?µÖR²÷¿æ­
$F0f¿âù!°:¿î³©æ÷UNASNone?ïEV&Zæ3?¢Õh̤P?—U;/{Ï¡?¢Õh̤P?ê¼Ss¾?ÅA¦Óé̍?ų›'1	?ÅA¦Óé̍?ê˚="Û?°JvJþå?Äїõ¬•?°JvJþå?íD$'@aš?Ÿÿ¾g?µÞÛîØÚ/?Ÿÿ¾g?ëˆÚç폐?½´(*z'?Áܔ`IÁÀ?½´(*z'?߇Be;?ÓfŸÎ´Oö?àw<^Íb@?ÓfŸÎ´Oö?è¨ØsÉü8?ºoþ"n©?Í\ž0Ø ?ºoþ"n©?áj= kè(?Á‰O»eW"?Ý+"¿(/°?Á‰O»eW"MIXED4FGL J1818.5-2036¿±â+ÂqAEÀl²
.À9ŠºÅ­À:Š@aïß!@
uΎBù@¢ÍbJ?ÑEäü"Ì?Ð0üw?ùúYÍÑ°?û輻@-?ÑE0¡2•)¿ç.yÖ¿èÿat¿ì<ø¾îì¿Û¦¾%6™¿ãi¸ËŽlUNASNone3FGL J1819.5-2045c?ëÏ^Ä;?Ɓ
dJ5?ÀÃþ‡"ï?Ɓ
dJ5?ëDd>Õ ?Ã:ƒ£Qî?Âîo«Ç€?Ã:ƒ£Qî?çà‡C£\?³hV"{?Ð>ñx¹áI?³hV"{?î>³ÊGah?'m6$¯UÑ?¬Ã\eÐw?'m6$¯UÑ?ì3C–O.´?À²ÅéÈtè?¾eãM†Šb?À²ÅéÈtè?φ†Äw58?Î{õ´¬?è^Nâ2²?Î{õ´¬?ä	¦¿Ç֙?¶è­}{?×첀pRÎ?¶è­}{?Ü;=nܒÏ?ÁW"ŒØý?áâaH'¶™?ÁW"ŒØýMIXED4FGL J1818.5+2533¿ìœ‹¹dÄ@2$Édb€(À:>"i®ðCÀ<ôËÛk@ƒ¸x¬äû@é/n'"š?ÈHLŠr4P?ҋÃbjÙ=@ޓ@ºs@Š]sùvú?äþÍûÌ¿à)F Mgè¿é±'IC?ñ¿ç-'àAõ¿ì`½¯ùWo¿ïþV²"<cUNASNone3FGL J1817.7+2530?ï_öåBÿ?'¯¤»H?"<ån?'¯¤»H?ï0ß° ¼?¢%¤Ð0?™ÿdÔ~‡?¢%¤Ð0?îá™VÂsF?"/¿`R¦?¡æj"´²™?"/¿`R¦?îÞ¾.ye?[ýÙÆñ?¢µ1??[ýÙÆñ?ë5Dúþ/é?¿[ÝЙú¬?Ã*ì@^?¿[ÝЙú¬?ê›ð5Ó2?ÄÝâxŽz?Ő?¯(³9?ÄÝâxŽz?éßÔÊOÍ{?±+1[<²?Ȁ¬ÖÀÊ?±+1[<²?矺½ÖÄ?«°ÍÔéä¦?ÐÀŠ"Ràx?«°ÍÔéä¦AGN4FGL J1818.6+1316¿í@ü(sÖ@*fZUÖÀ:h«=0À<€à,@ÐøÇÒg?þ7Tð]?ƎNâ¼"[?átÝ!®¦q@mÝS,Î@¡ÀM|€?ØîBþ­Dœ¿Üô[艿ЏÊB®Ñ9¿á›þÝÁ¿ïó6>¿ïva0FšUNASNone3FGL J1818.5+1320?ÕDcËñ€?Òð(ï.îÍ?å]ÎpÀ?Òð(ï.îÍ?֧ȾA¼?ÊVêÈ`W?䬠ß!þ?ÊVêÈ`W?Ùšôb'ò?²îߎáÓÇ?ã|²…ζ‡?²îߎáÓÇ?ä¢|Q_C2?­)¬øv<Ö?Ö»]Ay?­)¬øv<Ö?±ŠÇÆÊ÷'?­Ý¤%,Âþ?íΧáèà?­Ý¤%,Âþ?¬©…#Y»!?¶ ïô[?î5g­…¬?¶ ïô[?ƜC͵*?±ÚïS6=<?êXï'µz?±ÚïS6=<?Ån\ ×?«Sö´=9?ê¤hý;÷Ê?«Sö´=9MIXED4FGL J1818.6-3206?çïO¦†gÀŒ†‹ŸÜÀ:#R©@À;Ûo¼P}Ç@—%'Ænd@˜{0›©?ËJ3•XÂ9?âîA'šÈ@å	9d¥œ?ÿiÅHŸ6?ïÌ¡-â'Z¿¬ñu?
e¿á±Îyu6ä¿è™¨èÁõÙ¿ïú×lbÿª?èøª O€ÇUNASNone?â…\¤¨k?ϖÂd>?ÚõFÞ¶¯)?ϖÂd>?Ѳ'o…žæ?ËÀqX̎¨?ç&ìH=0?ËÀqX̎¨?à»ƒ?´ĘT;?ßÎäˆÄùÞ?´ĘT;?ÖÉÆçŸOÖ?±Å«¸ŠË?䛌0X?±Å«¸ŠË?Ñ\1aÕe«?ÌZ«×"ªê?çQçOM*?ÌZ«×"ªê?¡úZ¨à\?±¿XÈ› ?îàZU¶ëº?±¿XÈ› ?¹úçT `?¥R¾õ»ÜÏ?ìÀ£5{ô?¥R¾õ»ÜÏ?'fýM
Èí?'n_Km{S?ïlÈ`—ù?'n_Km{SMIXED4FGL J1818.8-2255¿ì
P#êüõÀ0U¸™9"À9×	—XvºÀ;>|2€…Ì@š¸ý·ü0@÷GMœk?аiϘ?Ò «†+(@wºÄŒŒk@¶¤¬È"?ïɯa!¾¿ê~Åý0¿à"7É
û¿ãÁ9ñ"U³¿ï÷Q۔欿ﴟ¿x{gUNASNone?îuðG%X?²L'`Á+œ?®x ÷B'~?²L'`Á+œ?í^.Ü·P?·!µÅÁ?µ‰E{Š?·!µÅÁ?ëñíB¼?¥¬ÑMȲL?À8I¿Þõ?¥¬ÑMȲL?í`ܻϛ×?"›åޝ'þ?´ù#¨âÉ?"›åޝ'þ?ä9"}(}?Æ¢&äèš?×ՌÙ¯?Æ¢&äèš?â]ÙÖåCU?ÑøìîÞÎ?ÛDLR5yV?ÑøìîÞÎ?âäI¾îpi?¸2yÚ-?Ú7l'#.?¸2yÚ-?âH'ðà¨L?µ«CWq»?Ûnú>¯h?µ«CWq»AGN4FGL J1818.8-0828¿îiýÌ#Ò@
\‰ô
(xÀ9e(ÃnÀ;=ˆ ËR@¹·_­@Sœº¶?ÇCŒ^?Çãv‡pÍ@7}_§/"@"؊ñ
?ïàƒ˜¦T"¿êF]ýŒ2S¿ãq
‰U~¸¿Ý:(e#ñ!¿î©"ÿ+Ý¿ïæítãìUNASNone?ëgÂÆRy
?À3Íl¯Ö?Â`ôæ¶Ê?À3Íl¯Ö?é¨$e©ÁÊ?ø î7+?É_niXøÙ?ø î7+?ë"€ÝqF?© ×~ì?Á¯ÅüŠ:è?© ×~ì?뼡BI?~? {i4¥bË?Á
zöÛ	? {i4¥bË?Ҏç~ÔÇB?ÈG]ë RŽ?渌@•œ_?ÈG]ë RŽ?Ö¦_A{m?ÑRÃjè?ä¬ûÐ_BJ?ÑRÃjè?â=*¸b2?»©:1»J*?ۅªÄ;?»©:1»J*?ÛB_I?¶I(c²"!?â^Ð}[ur?¶I(c²"!MIXED4FGL J1819.0-1203?îCÐÒjñf?ùé5¹qÀ9h™YùÕÀ:"Š.‹@ÖÿU¶ú@)ú}	@?ÒÐÏ:æ/õ?ŁÛw_‡û?öýŒ£ ?ûe¦MC?ïÐN+Ý¿éx¦¿òÉ·¿è ˜'[Ýv¿éþ_
¿âˊw½¦¿¿ïûï< UNASNone?í£€s`}w?»·ê‰îx;?²ãüdŽ Ê?»·ê‰îx;?ç'ö?©?Éþ£?ÐÛÂ߀¯?Éþ£?èڇ1Úe?±'r|3?̕ã8–kß?±'r|3?ìµßž>LŸ? aƒ…^Ð?ºQ
›? aƒ…^Ð?é¯3JkoK?Ã%Š?ÖÒ?ÉC2ÖRBÔ?Ã%Š?ÖÒ?ËGA¨@üJ?͖šÒë?é./•ïÀî?͖šÒë?æ%EBïÅ?¶"WÖ;ó?Óµuz!üw?¶"WÖ;ó?Ö=ó4Yg¿?¾'t²Ä?äáeÓL ?¾'t²ÄMIXED4FGL J1819.3-0935¿ÔLò¨ç"@>°YÏ/À9n*†¼GDÀ:Ç'*ç4W@áꛔÆv@‰1‡aˆ±?жšÙ4º?Òiëáºð@±îúôþD?÷L³è$l?ïÿ••_x¿±úfch¿êñ´âg¿é¿ü¿ç׏³•¿ïÿ!é^ÓËUNASNone?ìhö©j(?À¶°7¸Ž?¼¸J´¯¼?À¶°7¸Ž?ÐX­>ɳ?Ååáñ¢E?çÓ©`ó&?Ååáñ¢E?è`Ñ¿$îw?²À‡>—"C?Î|¹lF$?²À‡>—"C?â·tò;q?²L:?ڑà‰?²L:?â8Ùº¾NÒ?ÐOP†fr6?ێLŠƒb\?ÐOP†fr6?˜ù'º'Zl?­I§ÿ6L?ï86Á÷Ëm?­I§ÿ6L?à}œaä»E?¹Sõ&Á?ßÇ<6‰v?¹Sõ&Á?°rA`fã?›Ÿ?²Ø3?íñ·ÓÉô´?›Ÿ?²Ø3MIXED4FGL J1819.4-1102?éÿ)M×#h?ÿ_ì»"À9¬m&SQÀ:žÄüô²Å@HÛìû@~@RiÄ¿¸?àôC3[w?ඥxÊìù@ûç¢;(Ë@£;Xñ‰¿ïðÞú̺X?ï7ÐQ¿Ø'k>gnÏ¿ê'ÂIÇI¿í}tՔòk¿é"[å$xUNASNone?ՔcÁ½Çn?Ñ©µž»u?å5Î!I?Ñ©µž»u?È,£lV?}?Åò|tÅ¥?éô×$êp!?Åò|tÅ¥?὇NñÞ?´oO"èd?܅ØñbD?´oO"èd?ݜ)VÍ?¹I'æL$Ç?á1ëÀT™?¹I'æL$Ç?•ñµÐ·?©?ž†«dÏ?ïPrQ^Êï?©?ž†«dÏ?'Ÿ'Ñ\4?£ì±Zà´&?ïkqN¡Ï?£ì±Zà´&?Ê´wÖÑ2?².ÜS['?éRâ
K³]?².ÜS['?šËÐÐô™?'±)k#ß?ï)¡yŒÞË?'±)k#ßMIXED4FGL J1819.9-1300?ß9Š/™J¿?íØ⟜èÙÀ8Ä,5èðÀ:BÁE°
@ÎÍ&8ú@×6žË2?Óí¶Üöe¢?Ѽ)çZ?ÿÄô@¯¹?ùŒ˜êS¿ê÷–¤ò"0?ÝîÅû¢MG¿ëõÄÝëB¿ê¯:J~©S¿àvÎ}üÛ¿ê¬çŸaÑUNASNone?èr\²?Ѻï6¦|£?Î5úõù8?Ѻï6¦|£?ÕÆgánM?ÌýSŒ]à ?åqœÌHÙ?ÌýSŒ]à ?á<£ïÞʦ?¶½é½Wë£?݆¸ Bj´?¶½é½Wë£?æT-©'ùf?¶øcÝjÁÏ?ÓW¤­°
5?¶øcÝjÁÏ?à;Ò°€T¾?ÓÒâq_úÎ?߈ZžÿV"?ÓÒâq_úÎ?¡IEH}€?²ö|ö*&5?îëk«A.@?²ö|ö*&5?ÜۓP̘—?ºÆ$ŏÊA?á'6W™³µ?ºÆ$ŏÊA?­(ߑ-`ø?¦J|šÃ*Ü?î-r¶01?¦J|šÃ*ÜMIXED4FGL J1819.9-2926¿ïÔ#FÖqÀñˉ֮À:ª3DÐêÀ;Óà{Ö:@˜p¤ý[@¦k|OÜ·?ÅÊE
K3?Õ[Á<ëÙ@g/3Ê1è@AyúíÇn?ìvµ~|‡»¿Ð—¿ú¬Y¿å7ÌÎû¿áFJÂpþE¿î^%"ôÆç¿ïÿÿ^ðP`UNASNone?ë©W‰°?Àö'ɐò?ÁZ¡Û¡?Å?Àö'ɐò?í
®qöp?¸ 'š‡?·Ç'Ž(}?¸ 'š‡?êΈü4æ´?©ŠÍ
_¯?ÄÅÜ,e0?©ŠÍ
_¯?í"f ·´Ñ?'žÛ¾P^ò?³\Êû@s?'žÛ¾P^ò?å¢g~>tZ?Ë$Çh<‡ù?Ô»1ƒL?Ë$Çh<‡ù?ÞpgðîÚ?Ò$a‰1í?àÇ÷̈"?Ò$a‰1í?âŠD ²¬?¹¦ìŠÏž±?Úëçv¾š§?¹¦ìŠÏž±?áÌÑ°Èpƒ?¸H²"º?Üf\žoú?¸H²"ºMIXED4FGL J1819.9-1530¿ïȼjæ#¿ÐWÁ•aüÀ9gLÖÀ;#ƒ×u.@FÞá¢G@í>" 
Q?̾­º¸Î?ïÿîbHÊt@Ôb^™éK?õ'{è-Ñ?å³ý">5Æ?ÝdZÝò%?Ѭ{ÃŽ¿èx²>@ÿîR¡)°Ó¿é©ÃGèÌÞUNASNone3FGL J1820.3-1529c?'&é]X?§Þ›K2sê?ïnȵ€Ÿ?§Þ›K2sê?¤œ?=ï?ªÌÍ7P°9?î¶<J¼?ªÌÍ7P°9?Ë¢B.<˜&?¬Ä˜êªÕÂ?éotpÙ÷?¬Ä˜êªÕÂ?b54{mð°?R
Ò2'ž‹?ïíÊËb5ø?R
Ò2'ž‹?‰íüÔC½?±¤¿OD·?ï˜Hw÷L?±¤¿OD·?t#£'Ó—?"6£!ý¸?ï×︊©?"6£!ý¸?§Æ…òß
[?™¹"Yëc#? ßÍÊ?™¹"Yëc#?cÉ@w®ö?®ÖøêË#?ïÿLáÚûå?®ÖøêË#PSR4FGL J1820.3-2646?êå®ðîÀÀƒëaãIçÀ:-îÉp!À;uñÀ¢@Óaš#Ø!@¢¢dCvw?ÔLÄô;Q?㥾/ûñ@©Ô•*™?þ"¡Û1"x?ïý
<(¥;¿Öy7¤\U¿éâL@Jrë¿êÞ́®Á¿ïá¤_Æ95¿éäL —©UNASNone?àìljAÛ?Ôx¨q½v\?Þ&pí}òI?Ôx¨q½v\?Ò¦'"t?ËÃÏ@M*´?欷znõÆ?ËÃÏ@M*´?é;ĈŸe$?«êJâ×o ?Ëí݂kn?«êJâ×o ?Ø>ÿÝÑ?²iÎê
)·?ãàž ?²iÎê
)·?Ö=nC™?ÐjçÑLH?ä÷áH¸^3?ÐjçÑLH?¤ÄmiÑ/&?¶,Յ÷ò?î³¹)p«~?¶,Յ÷ò?Øãå5Wy?¹Ä|J˜?ãŽ
eT~Ä?¹Ä|J˜?"Tþ
ç£?€¶_Ü_@?ïgWد?€¶_Ü_@MIXED4FGL J1820.7-3217?ç}saÀ wB™ØƒºÀ:"Ô+|À<WÔUWJ@$‹Å¦Ê?þÖË8x'?Ñð\žçaN?çmjW@KU}
Ú?ÿ§‡ Q»?î[õÊd?î±ã<zÛ¿ÆQ$ŠÎÑ¿àGóÿÁ–¹¿ìUŠÁ9›­¿â]ŸˆUNASNone3FGL J1820.4-3217?࿦¨Ã$¥?ÐWø$…™?ހ²®y¶¶?ÐWø$…™?ÔçHÏÃ?ÌîÎ>Æ?åŒ~Ûþ?ÌîÎ>Æ?ááVãwÅE?³ù¦õ€Þ?Ü=R9uw?³ù¦õ€Þ?Ô;%;—R?°Z&:rã?åâmqâ4W?°Z&:rã?ÕWo>7"b?ÐfÖÖ?åTH`ä=Ï?ÐfÖÖ?ª"ÅVXH¹?µËKßOÒ?îV³ªß3¤?µËKßOÒ?Óju¿Ÿ¾?¬‹p!€LN?ë%b?¬‹p!€LN?­xA-'wv?ž–âÈ>?î({í[©?ž–âÈ>MIXED4FGL J1821.5-2531?ê-aÉ.ïÀ&,ýxÀ:úmïǤÀ;c\Äüô³@àû­àÎ@4@^"àÍ?Ìj(è¬|J?ÉÙ¢Ò1f@8ݗl@íÚ£úñx?îÿü¿¿Ó½°d·9¾¿ê$'ýuE¿ßL‰°îIõ¿ìòSš¿ïÿ7ûþéUNASNone?ìjލÊ?È­µh_Ã?¼©Oˑ±?È­µh_Ã?ì'Sdÿ?¾"þl'	Z?»udÛ÷¸?¾"þl'	Z?í_mØdtc?¡³21€€™?µ'<nil?¡³21€€™?íN¢0R>w?–®!¬q9^?µŠî}nD?–®!¬q9^?Þ{¬ô•=¿?΋JmÙÅ?àÂ)…µa ?΋JmÙÅ?àhëõS?Ób¤¸±?ßÙ.ü(Y?Ób¤¸±?ã
%}›"Ï?ºöÕá.À?ÙåµÈÖb?ºöÕá.À?ݎ"ڗÝú?»aSŠŸ3j?á8?»aSŠŸ3jMIXED4FGL J1821.6+6636¿å4°k¹#@;ª% Jù#À;(o`àëhÀ<Öö¾7ޔ@ è¬Û•½l?ühžŸ'×Þ?ÃÈÃRЇl?¯©¢?g¹?íýú1@	ĺËÃbk¿ìÂmÎ9´W¿ïÿúâô?ïÿíUÙPi¿åØQÀ'ô¿»OÐ^
¿¿à^¨A}"ëUNASNone3FGL J1821.9+6636?ïÿŸ›CñO>úèù/s'?-B1B>úèù/s'?ïöŠ°j
?U±å·5~?RêŸkÂÈ?U±å·5~?ïö@"xP&?XEB¢b{*?S~זbx?XEB¢b{*?ïþií¯pq?ñŠ(Œâ*?)a&s϶?ñŠ(Œâ*?ïÿƒ%cç±?	6ç.S"?6£ð0 Ã?	6ç.S"?ïÓ¿Œ6H€?€ÄV(Ò?v 9ìjãØ?€ÄV(Ò?ïømeÙu?_¶?'×?NJl»°_?_¶?'×?ïý)HE5Œ?0©,»s(Ú?6µ½5ÌJI?0©,»s(ÚAGN4FGL J1822.0-3146?Ì6¨™ÍØÀ ySyú—áÀ:•¨þ'j÷À;ã)þK@ႁOù@4Ÿå
5s?ÊoEFl?§¿^5{ž?⦓}æO@>—…BI§¿Ú
ý‹["?ïþô1•¤B¿è@C=¿Ý'œdÐK¿ëëÌ!+HÙ¿y¹!/‹ÅUNASNone?ïÒ1›Ä?"/`n>qâ?vç7¿,xË?"/`n>qâ?ï´µÕˊ>?ËN¢™UN?'ÒŠŠʔ?ËN¢™UN?î™–‰~?š&²«Œò?¦n¶ž»?š&²«Œò?ï¶tôÒ-?hQF³Þ?'bÂÉ
 ?hQF³Þ?ï'oª' ?•&`FN´g?‹¤|·õ?•&`FN´g?ìùÙ[Œ©Ø?Àù »"ô¢?¸15%R<?Àù »"ô¢?í½æXA¾?£pÏ̶›k?²Í?;é¶?£pÏ̶›k?íí,aÃû~?¢(qûOT?°–œñà$?¢(qûOTAGN4FGL J1822.6-2502?ÙR•
mÒÀ½Û˜A«À:q7öçRŠÀ;…yB=K@ÞM¨ªY@´ì O*à?ÕÚ/¡XTÖ?à"Ìô9ù@Xæj,Å@°
©¶È¿â!֝l¿æð+¬V4À¿Üɀ2Wk¿æ®°:Ê¿ïÿϞcWé?äæ»@2uUNASNone?ì¿·Xtû?¼J© ¼'\?ºE?$X$?¼J© ¼'\?æ</ŒÄ/?Î/;¢—v?Ӈ¡Âæw¡?Î/;¢—v?é­ÅÚT}?¬ÇAë¯Ql?ÉH딖®
?¬ÇAë¯Ql?ëwü¥FdØ?ª
,_̜»? 
jæl ?ª
,_̜»?âü˜±´â?Í{ÕMú´½?ÚΜ–à=?Í{ÕMú´½?¿Ž™Ø¦L?ÇâE§K€S?ì,Äë=6?ÇâE§K€S?Ü
¶úR—?Àc·µcy¢?áùp¤'Öµ?Àc·µcy¢?đ­§m—³?µ–VŠy‹Ê?ê۔–$š?µ–VŠy‹ÊMIXED4FGL J1822.8-1118?æùóZ}ã?ñ&Y0þÀ8çíåÀ:TK8ãv\@±Õ>ì¥@ÃJ‡ãŽ°?Æ~Jž3Ý'?ÂƇÕvê?ý¹|X@2ö?ÿì0àr›ÿ?åxÿnw­¿äƒÛÂ3¿è%Ò݈ó¿å'úhçJ'¿íTvyÙಿïóܦ^£úUNASNone?ÝÐþ^®ûÅ?ÓþFÊó6?á€Ð¨'?ÓþFÊó6?ãùÔQrÛ·?ʊgF$x?ØW]H'?ʊgF$x?âÅ8#»yœ?¶ŽGí.¶?Úu¸‰È?¶ŽGí.¶?èÜw݇/4?«xèg:ªT?̎ ‰ãC1?«xèg:ªT?À-EH­N?ÁðIµ™ç?ëô®­ýÔ­?ÁðIµ™ç?Ä¡Ihv-{?ÈAÔÖÜp.?ê×­¥ât¡?ÈAÔÖÜp.?àøºD°?¸YµÉ%"y?ßÈ‹wܟ?¸YµÉ%"y?È!žÖobä?¯U.£µ?é÷˜Jd'G?¯U.£µMIXED4FGL J1822.9-4718?¢†:5=ËÿÀ.,ê(þ&À:cÞº5"À<6%ðT'R@þ 8¯žê@!%‰Õ?Ãÿۂr5¨?Ñ'ýž%ð@	N½ÅÈ̍@¡ØàVls?ëJ%󯏥¿Ý(¸ÛÔ&³¿ÞÊZâN¿+¿äÁtæX¿ïÿòɶ—׿ÉÅèª;}UNASNone3FGL J1823.2-4722?î5&ÔïÊÂ?°µ•_¹~/?¬­'±ß:×?°µ•_¹~/?ï"žA-?¡/SéVÞC?›¼Œ9"Q?¡/SéVÞC?í(:‡Cq?¢ÄQ!\{?¶¾+ÃÁúû?¢ÄQ!\{?ï!2'Ÿc?{ëª<7ì?›Ù»%cˆ?{ëª<7ì?ç‹(´÷e?ÇïœÛð'?ÑÌ鮖5?ÇïœÛð'?êˆv"ý¼j?ƅ¥ñÁ£Ï?ÅÞ%ì	X?ƅ¥ñÁ£Ï?ãZ¨'æt?»Õ./¾3­?ÙJ®ÜÄ3?»Õ./¾3­?é´yџ'Î?©w	|t}?É.¹¸Ê?©w	|t}AGN4FGL J1823.2+1209¿ïÆßëb@'eÿ'+¾ËÀ:Ó°QlÀ<ª¾
'*:@­B§šcC@œa½Š9ª?ҖÞ­?ïÿ¤%
ւ@D9ô"?ûfkâ|·¿ãÉ¢
cB¿âɹòÕu?Çñ½_œs¿éÒ¹
x)¿ïþdž;îÄ?¸xQJuoUNASNone?ƨ®
Þ©³?Æ2 ?êUÔ|ˆU"?Æ2 ?Á.ö¶]Ó#?¿0r…ûÏf?ë´BRh‹7?¿0r…ûÏf?ݍ
iÊôÛ?³Žç"´A?á9yK…'?³Žç"´A?»Þ"¯Ïç?¢6U¦k?ì"?­j?¢6U¦k?§V@NZÉ(?³Ø¯Õ¬Uš?ûQM-?³Ø¯Õ¬Uš?'×ý%²?™ÂïtÂ^?ïwçMÕB?™ÂïtÂ^?Ä)+ ÙÙ?¬7i³(à?êõµ7ɉ»?¬7i³(à?sœ\P½¤'?e)™ñÌ?ïØÇGZe/?e)™ñÌPSR4FGL J1823.3-1340?ÓþˆImºÌ¿½kW½VÀ7d_4Bý¬À9Ðè±.á•@VIã£Ô@0k_Êjó?¬b¡œ»­?ÏWŠý@Áæ??öÍþîˆx?êÔ½‡	Ÿ?Ó¸GD7<'¿à¤¸F-
û¿ã!½êÜ­¿ê
Ä
áj¿í¼ã`7"VUNASNone3FGL J1823.2-1339?•mû8Ά>?°d½LÓ?ïT&9‹Î?°d½LÓ?œ@ÍÍHÑ?¡+jCij?ïù'À¡	?¡+jCij?ÅtÀlþAJ?°õ@2,õm?ê¢ÏäÀo­?°õ@2,õm?xZ1xjÄH?e%"Ÿ–×?ïÏKjÇ?e%"Ÿ–×?€j©èc?±œòùo?ï¾U["¾Ÿ?±œòùo?n}UÅG0
?~UóÍÓ?ïႪ|@?~UóÍÓ?™žÿ¿P?˜*%²_ ?ï3ôE&?˜*%²_ ?·¿ðý+?&¢ÐÀ¡·?ïÿGJKˆ?&¢ÐÀ¡·PSR4FGL J1823.8-3544?ïJGgPNÖÀ$³H+è¼À;!<ÝÖàLÀ<­‰;}…@³GC¸?ÿŒèæÞÆÊ?ÓÒ\Ä&5?å±	!ç±U@HŸž–Xœ@µy'=/?ëLѿкî?íVˆm!k‹¿Î-º"{*¿àò÷ÙÀÑ¿ïÿŒri©è?è»K€1ÈUNASNone?.œS;?«ž[Mê«?¤‡íË0V?«ž[Mê«?í/7*?¹ƒŠèÀ?³ö‡"ŽÝ?¹ƒŠèÀ?ê
ƳòÐ?®åÐV~˜¶?ÇÈå04¿ê?®åÐV~˜¶?îJy("z¤?'ó:ÛÚB?«Xmw¤<»?'ó:ÛÚB?íLJ701»?µ#ÛŒ?±ÃÆF~r)?µ#ÛŒ?àã;r-*A?Ñ㊕š±?Þ9‰¥«~?Ñ㊕š±?ÓºvÄ¢?¼°¯4á?æ"ĝÿ.õ?¼°¯4á?æU§´º\]?·'EƒSe?ÓT°–‹GF?·'EƒSeMIXED4FGL J1824.2+1231¿î;&L	ì@'Fd+ùƒÀ9ùžã…uöÀ;°öüK?™@²è @¬6|"ÏU?Å]b[¿ÄQ?Ȓ›ãö´þ?ýF©î@tÂâ¾%À¿ïÿ²'ž«Q?ïÿú Âî'¿é3¼$Þܚ¿çn¦`ýEæ¿ïõpŸÐ?s?î"úÎg׀UNASNone?îDmôø†?º2€ùÃ-š?«¹ Á˜Eš?º2€ùÃ-š?î©sö`³¹?°õ¡Ñ»7é?¥hÀ˜<öv?°õ¡Ñ»7é?íût‡D
?œf5 ð§?°'äZéø°?œf5 ð§?ï5"àeí?'œûbß6?™[£ö±ûû?'œûbß6?äG8Ï»zÑ?їâ–õE?×qŽ`‰
^?їâ–õE?ärvKz–Ž?Òü&cŽg.?×i
Òä?Òü&cŽg.?ã¥èÛ²T?½.-áuâl?Ø´.H›Wè?½.-áuâl?çOåÌU·?¼Fjr"ˆ?Ñ`4gT'Á?¼Fjr"ˆAGN4FGL J1824.2-0621?â9­_ô@ÐD¡À›À9F¿'țæÀ;Òê šª;@ݕܠªZ?ú7#¸kì¸?¾‰/¿
l?ãaŸËŒÜ@!gÛ	¦qï@>Ašÿö¿îYÀGƒL?ïñs	â×Ñ?Ä+üŸã‹¿Ô×~×v¿èUæ¼b~¿ïÿÿ" 5•UNASNone3FGL J1824.3-0620?"ƒØ#,?'²x!t¦?ï»uðÙ,¾?'²x!t¦?žR¥Â±f?¡žiTZßÅ?ï}j¨¯%?¡žiTZßÅ?Ô|Ì\˜	?²8|uhÚ+?åÁ™Ñ³ø|?²8|uhÚ+?¡Ö•°—<?‹Æ÷ܱL?îâžÆ²´ü?‹Æ÷ܱL?†Ã'nî?'o†±ÆD?ï¤ó‹8¾õ?'o†±ÆD?pԚÃ|^?'®C£Ü|?ïÞVËÏÝß?'®C£Ü|?ÞÆq«ü?¸ÿ¶ƒ/+?àœÇ?*s'?¸ÿ¶ƒ/+?\ÞYBօ?R²ñŸä
;?ïñò3Â-?R²ñŸä
;PSR4FGL J1824.2-5427?à1qo·|À2Œ`Ëò²À:[ùæ
‹tÀ<‡²ù¼ïà@¤lŸ:˜W?ü~CÖ[?ŋ)ÿ­Ê©?Û9»n€'@Äq´xB1@ð¾'u³¶?îy;àÖÄó¿Î¬xCˆ–¿ Ó¢ s4w¿á™i=[U;¿ïêúêíID¿ïÿö$´ë/UNASNone3FGL J1824.2-5427?ÝZ‹«fÃ?ËŸ}øm?áRøº*LŸ?ËŸ}øm?çDígeÚ?ÆkBc|Ò?ÑvÞ%14M?ÆkBc|Ò?ÙIo!×t?³"°EañÓ?ã[HqoF?³"°EañÓ?è" ‹Qû?©?Êݗ?ͯ}Óâ¸?©?Êݗ?°p}Ag?¯=ÿ] u?íýð\7Ó?¯=ÿ] u?Ò×æíp—?͆Þg:2?æü"‰G´?͆Þg:2?²M¾xþT?£å´™õ?í¶H0ÆFv?£å´™õ?Õ=ÿF"}?µªôÎE3@?åa\µýA?µªôÎE3@MIXED4FGL J1824.7+2403¿ÌVñ9¤Í@0HÙºÀ:œÑ¦PaAÀ<\G4q÷"@Sûª°Ã?þh¤~Ïé¸?ÕH 'Áç?Ù¯}HÖ@‹ÔÝ<†™@a4-.6t¿ï§x_7H?åì¡~ji¿Ý¥a~õÿ¿ã'&"©x4¿ëȽhÖ®¿ïÿöÅĚÏUNASNone?îéy}X-?¢ñpþÂS§?¡hh.ž–1?¢ñpþÂS§?ì—Õ©ë u?¿Jk!ûÂ?»AR°¦üY?¿Jk!ûÂ?íZ^é‰"? {£IÒ¤+?µ-¸}ß? {£IÒ¤+?íFÃ#^\Š?'€"?'[?µÉææÄé«?'€"?'[?éøŽ¼ÆÅL?Áå"oUoÀ?ÈÅäêÑ?Áå"oUoÀ?ã±Oœ†š?Ñïõ©Ãeù?؝`ÆòËÃ?Ñïõ©Ãeù?çñm*¥Åø?´½Ãþ¶?Ð%ª´t?´½Ãþ¶?ãÞ>"}dž?¸-Îïa®8?ØC'Ù6Ã?¸-Îïa®8AGN4FGL J1825.9-3153¿¨îñãþ.ÔÀ"ÄÞÁÁ×À:"×`¤…†À;¾k#d‰@'ZïÅZ@ù4ºð!?Ïh`fþ?Ò@âô,@QáŽû°æ?ü†WÕÔÞ>?ïœÈùµ½¿åX=˜çÿãó"Çz¿æ:´ÒD2¿ïû]èHS?~+VUNASNone?ïS4":¤? ¢é‡j?•™oàà"? ¢é‡j?é¥ç¿±6?Çì²6Y¿u?Éha;ƒ(?Çì²6Y¿u?ì-ô5Žq?¤J%øi?¾[öSŒx?¤J%øi?ê5LKÑb?¨¹¦ÍSŸ?Ç*ÎÓÀºx?¨¹¦ÍSŸ?ìRsåÕÝB?¼@"M…ã?½l`ÑQò?¼@"M…ã?Åyõo-__?ÉÔ	­þ«?ꡂ¤4¨(?ÉÔ	­þ«?ã
.x•?·(_žå͔?Ùåé£óÖ?·(_žå͔?ÈÀ&>`Ái?´º¿ÔÎ?éÏöpgϦ?´º¿ÔÎMIXED4FGL J1825.9-5614?éùÕ	°À2ì|ÇÑ»IÀ:tý£.mÒÀ<W¿Úv@"¹._cé@\á>iÈ?Çòfh?Àkj1L(?ðu'a¼³z?þ±Naaï´?ïþ'¸«­˜¿äé5¹pß¿å¨tþ¯ž¿éžƒ¾ôÚ¿à2Ô¿ëÉú?KÅPUNASNone?ïû§D–̤?:Z¾,Ž0*?Abìñ•M?:Z¾,Ž0*?ïÑģħ?‡f"bšBÑ?wtÈê `?‡f"bšBÑ?ïÊN¹‡±Ì?t¨œÔî?zØ£C¶>
?t¨œÔî?ïØþ¸y¦?YPê˜0?sù€™tY?YPê˜0?ïòÀò3?Wõtôç"¯?ZÂ$ªß?Wõtôç"¯?ï\IØø:u?¤'Pèý?"vÄ݉e?¤'Pèý?îøX@ÞÂn?—͏\­>¸? z{íÈV,?—͏\­>¸?î…"@i?•Z4olv*?§­Ûùn?•Z4olv*AGN4FGL J1826.2-2830¿qm¬wâüÀXpƒڑÀ:zyöf#KÀ;åµWeA£@á]'£]@\¢}méè?ѯä^¹É»?ávU⊤3@«4<Ëb?ó|¥³Û?ï";ÞþR¬¿Ð»ÙÊâ¿é¦î¡ˆÑJ¿âTÿ5Õ¥¿ïÿþ½à ¿?ïÿÞr¾"UNASNone?Ï7¹0$û?ÏY3BL«ª?è2¿3öÁ?ÏY3BL«ª?ÒØÉ7õm^?Ì@Oª¦öé?擛dIQ?Ì@Oª¦öé?çt5J0?°´ñӆ>?Ñÿ•Ñk¡?°´ñӆ>?ÛWúº"0Á?·2Hµ»5?âT¢¶gŸ?·2Hµ»5?ÎÃA¼@–?ÏZBt¢G?è/ïÚ?ÏZBt¢G?¡Eß¹1¼?°B®ð"²l?îë¢C¨ï?°B®ð"²l?Ôý÷VÕá?·º)« ßÜ?åvԕ?·º)« ßÜ?"‡Y›¿É
?‰°77}.?ï[Å3Xûw?‰°77}.MIXED4FGL J1826.5-1202c?ëN9
_0Š¿­Í¶<ù–ÁÀ7þ)›Ú¼zÀ9îõì@ß·Ú@¹Æ_ËA²?È
Áúá³?Û«;³´M@ϱÀo?ûFîK¢•Â?焓xhҿՔÌÀ¸ln¿æwóÂî¿ìNwÇ·º¿ïÿþÐñ?íì|*	üUNASNone?ÚaJUÂ1ò?Õ.æYP1?âÏZÕç?Õ.æYP1?­Q½Ÿç?¯Íú"¢ø?î(
ä=4q?¯Íú"¢ø?Ü1òrñ´?¶¹HIa?áçƇ}&?¶¹HIa?¼ÄäqÀGê?£Mß8g?ìgcqÇ÷?£Mß8g?Öe¯Õ£¾"?ØKRƘ͎?äÍ(. ¶?ØKRƘ͎?u¦âÃ\HD?ƒò÷ސE?ïÔ²:`Š@?ƒò÷ސE?»hµ'û"Ù?¦˜½«»'å?ì'éO e?¦˜½«»'å?X»1½éåI?O¯ê"UA™?ïó¢gQ%•?O¯ê"UA™4PSR4FGL J1827.2+4303¿Þô¥Œt¡@6RÿŸ‡ð$À;$;ž;¿ÊÀ< j0'|@áH—žl½@aÙ¿#–Þ?Ñ
#hú?ÇTÒª²E¸?ôu"‡!œ?û[Õ@Ž»o?ãìá•0Ô¿êi‡]æJ¿Ç9`¿Û/dý/Á¿ì=#vý_¿ïÿŽ@)çUNASNone?ï«G@}Àí?…ݲª'?…./ñ½ÐŽ?…ݲª'?ï *-Ë?"3Ÿ4{AF?‡õtÐ{Fâ?"3Ÿ4{AF?ï4<–šqí?&,>€?™xm,±Âc?&,>€?î֟À5uê?hEEÒŧ?¢–ù9h?hEEÒŧ?ïXM>L@ö?ôƞ±ò±?"öX-àÛD?ôƞ±ò±?îFZ漞=?³?SW³Œ?«šQ–ÉÑ2?³?SW³Œ?îF1J®WŸ? Iƒ®U%g?«œëT>Ÿ? Iƒ®U%g?êp˜D–Ä?§"þméU?Æ=Ÿ®í¤ð?§"þméUAGN4FGL J1827.5+1141¿ïß¹ÓJë@%ô‡ü¹$À9ȄÚ`3À;÷é"mé@@ö¥8^@+¢õÚ?¼±4u¶?ÖÒóW{@v!`¢Ø@Š¥ÜÈîF?ïøTÛ#§¥¿Ø*¬¼aË¿Ü¿+Žúg¿áÑýžPãr¿íê¬"¢º¿ïÿ¶>@£UNASNone3FGL J1827.7+1141?Æ.[Ñ"?¼Òì™q?êty)¼ø?¼Òì™q?Ñ´Vo‰Œ?Æ$4l)?ç%ÔÈ;:?Æ$4l)?ÒÇ㸐n'?³ïaM•¬?æœ#·È·?³ïaM•¬?ãƤ$ôp?®Þ®ÊÎÝÙ?Ør·¶Ý?®Þ®ÊÎÝÙ?Œ=ÀËyÊù?‡¥pT‹N?ïü¨Ý"?‡¥pT‹N?¡âQé2²P?¬óÄvPº?îáÚá–+?¬óÄvPº?¡rýãµ?™ãÂwô?îèÐ"¨$?™ãÂwô?À2¯]XÔ5?¥‹w‹àp?ëóT(©Êó?¥‹w‹àpMIXED4FGL J1828.1-1312?î'(LWúñ¿íƒîÓTPÀ7酵·'À9s7+æ7Ø@"ž >¤V@mPes!?É!Þ!3ˆ?Ðå%ßÀX?þxøŠ.Ã?úaÂgÄ
¿ápÈà.(‡¿êé/~¿Ä¿åÝÐ?ÈíÅ¿é'9@=‡Ë¿íçÀn¹¿ïÿîbHÊtUNASNone?Öɹ=_N?ÓÃ
tyù?ä›#aPtY?ÓÃ
tyù?Ö(tÁý*?ÏÓÙ看?äëÅôŸk?ÏÓÙ看?ÙHµ<£»?µÄÛ°5)'?ã[¥añ."?µÄÛ°5)'?ÛþÀb<?¼yúŠþ©Ç?âpŸüÎâ?¼yúŠþ©Ç?یNK¡?Ô\êÎâÉ?â9ôØÚw/?Ô\êÎâÉ?° ¤ªã¦«?¾1¯`¼iŽ?íûëj¿?¾1¯`¼iŽ?וaX­Ÿ?·3'ô"}?ä5O~S©1?·3'ô"}?œBvìR¯?'šHzZI?ïìH¬ÛÚ?'šHzZIPSR4FGL J1828.2-3252?ⓄM›ØþÀ#˶ˆ½©CÀ;)mã2iàÀ<¬ÝpÜ@ûàÖÄó:?ú®!ÛòÚ?ÕØá-,?å'Á)h¯@
`9[k`¡@Kº5›mY¿ïߕÇ}³?ïÿ;F',¿ÊŒbN~¾¿×<(¿íwi¢ò‰¿Óã~T™µHUNASNone?ïÀa»ËŒu?ŠŠiJÓU+?Ï"{Uº?ŠŠiJÓU+?î[صR £?³k†[BS´?ªBt¬•ÃÎ?³k†[BS´?íQEGæQ6? jqbЯ?µuÕÁ©]P? jqbЯ?îXbo`àë?íÍ­°B?ªyÙ^<M?íÍ­°B?ï'2cÄ9o?™ÏuVjÜ?‹³g¢ÐE?™ÏuVjÜ?åÏ"ÂD*?ѳ­"ÖÄÑ?Ôaº{w«Ä?ѳ­"ÖÄÑ?钊å)m•?³^®É…Z?ɵÔkZI«?³^®É…Z?鿸ã>†×?µÿb&Ìٞ?Ésä¤?µÿb&ÌٞAGN4FGL J1829.6-2545?Ô9rINÀ"`št‹À:unF.¸zÀ<HåC¼s@ÓÜäòÞ@OC427?Ó-&ÿž0W?ïþ
hø@!G'R?ìђ&ç( ?m¿Ýß<;±'¿ád¢A¿îqkGv·¿ïúYbqå ?ïå«@
11UNASNone?Ó®5•?җ"|?Û?æ(üe85s?җ"|?Û?Á?[EÝ?œŒjS}M?ë¾ð).ˆ»?œŒjS}M?â[#(ñ]G?²ø¾xcM‰?ÛI¹®Eq?²ø¾xcM‰?£Búhy·?'©ÎVK?îËÐ_˹õ?'©ÎVK?ÎtR"©"Ü?ÔI
xmû?èbë^՚É?ÔI
xmû?–Ÿd9~?¦•Òß?ïKÞaÔ?¦•Òß?ÆOc=oª»?¯9Y€Õ?êl'0¤Q?¯9Y€Õ?MËøšÏ>ö?D¤r^ç8?ïøÛ¢S?D¤r^ç8MIXED4FGL J1829.6-4310?îíÅãÀ-Ǽ"ŽÀ;>@ÈG,À<Ñý¾Ý @zú*O	@Ôj»_¼ÿ?ÔãÌ"'áÇ?ëÊÝßCÈ@	œ?,eº?ÿSƒþ&áì?ë©È»ÆL¿ã‹¯Rhƒ¿Ä¼=Þ\í¿èwsÔãòƒ¿ïÿþÞ÷¿ìÌòÂ)ۜUNASNone?î°
b'ñ?¯(ÃëîX?¤þß)×Ðó?¯(ÃëîX?ìŽüâê?·ãmU^z`?»ˆè¯+|?·ãmU^z`?ì3ìÙ)þ?¦á4€î°€?¾`™6·?¦á4€î°€?éDÞx¾$?«øï~HG|?ËÂì†o?«øï~HG|?ìJ^%LJ?Á¬í<Ì?½¯åÑÃÆ?Á¬í<Ì?áiÍJî]8?О}¬Ü ?Ý,ej#E'?О}¬Ü ?æ‡ËbP?»1²]œ?ÒðiÇ;_Ê?»1²]œ?՝+¥ÜYC?¸¤xtϓ?å1j-Ó_?¸¤xtϓMIXED4FGL J1830.0-1515c¿ÔÁ,íÁ0"Àc÷¦•*ŸÀ:IVH1ŒÀ;Û¸øÚr@"k³bmˆo?ÿXß_vˆ?Ÿˆ¨}®-¿¸;øÿ…±°?ñ>Õ'å!@Þø4Y£à¿âž%"ôÆç?î{P}ñÈZ¿é|í'hr°¿àòG°˜¹ ¿ÔɎÿ·°±¿àz 9påUNASNone?ïøåŠïîÌ?h™)ÆȲÔ?LiÓ§oÊ=?h™)ÆȲÔ?ïCjø5J)?¦CŽè>,?—' õçô?¦CŽè>,?ï¯U;#u?"wè\èÁ?"<*»Ýì¦?"wè\èÁ?ïߐØĖŒ?`,lFíÌ?p7"'
ô?`,lFíÌ?ïÑú ¼ðÙ?zŒr5â?w¯¢çku?zŒr5â?ëåøz?ÄÇ»|y?Àhõ¼²?ÄÇ»|y?ïIù¯j"?—ÁŒ(¢'?œÖÀÃ3ƒ×?—ÁŒ(¢'?îò
—õF?™*&B™x? ß&"`•?™*&B™x"AGN4FGL J1830.1-0212c¿ï 
èÌ@
×õfI
À9?|–S"üÀ:́I@»²@Uñ3^|7@]gº#}?Êu¶e':Ø?áPVY¨èÂ@¥Õo2½Â?üLH=0?îˆ@
²
ª¿°†òÍèU¿¿äF­czù›¿é³©Xb˜¿íÙä"rÁ?ÐyM>!MØUNASNone3FGL J1829.9-0203c?ÑÍôg?ɓ£;êøî?ç|™þzL?ɓ£;êøî?³Ýc©	ނ?³'A"‰Š9?í"SŠ§Êp?³'A"‰Š9?Þ=F¸Ý<î?´ƒËeQe?àá\£'a‰?´ƒËeQe?đ§÷o&˜?£äE¤Z?êۖ$6Z?£äE¤Z?¡À*Ú¢?¤EAB^'?îãýRHÀ?¤EAB^'?1hID¶?ŠÞ=Þ[?ïÁœåJêV?ŠÞ=Þ[?±ºØ}ùã®?Ÿëd>MU?íȤðˆ:?Ÿëd>MU?q:)É1t³?^Èrž\??ï݋¬¤–Ö?^Èrž\?,PSR4FGL J1830.1-1440?Èe*`?Ÿ—ÀWµäRûPÀ:%ý®(`À;Y.Œ…¡@!a÷q'á@èû"°ý?®_+‰›Ÿ®¿¹%ya?ñK&õ7O"@)$衦?îçYޘ§¿â{ê'Ù±¸¿àÒZu—[Ò¿âðóˆ"xÑ¿åIׄ¶³†¿Ð?"$ghoUNASNone?ïìRPÚ¸ô?_—y‹±?c­¯êô‰?_—y‹±?Ï<"¯?¯òѓ6ý8?¤g"¦a	?¯òѓ6ý8?¸®T?ˆ"þ
¡3?‹'Ɲzþ?ˆ"þ
¡3?ïq‹ ²'?x¥5Œr?'΋ä†D+?x¥5Œr?ï'[êD?ˆmA½]Ÿ?i=ÿcÂ?ˆmA½]Ÿ?èã)*Ï?!?ʱä…~J?Ìs[TÃ~?ʱä…~J?îúÂ÷6ð?—¶^6Ç0c? SЌŸá?—¶^6Ç0c?ë¡
珛¿?¯ô`¶È?Á{ÔaÁ'?¯ô`¶ÈAGN4FGL J1830.3-1601¿ê{½¿ØaoÀ¥Ûüëx‰À;;?´JõÈÀ<«Ü'<®@&~Ç!' ÿ?ò(IDíoÛ?Ôπ0fû?ÂÏôŸy­k?æÒÎn|@Š'‰)ßÍ¿Ì[/ürù¿ïúÙ_­9µ?ïò×ùP¹V¿ë¤šéû±½?åg*¡iFÁ?ÎUå]gUNASNone?òŸ?µµ‹ž¡nº?‹?î4:?µµ‹ž¡nº?ï†^1"?¢±ÇŸÒæ?Žh{u*þ?¢±ÇŸÒæ?ï'ÂN½?‡Ñ?ѐѫ?‹¹Oi
4Ö?‡Ñ?ѐѫ?ïù9kà}?JÒ·¿Ó[k?KT#Üè?JÒ·¿Ó[k?ïï+ÆϪ?gæ*,«…?`Ô9]°¾†?gæ*,«…?íhcxH\?ÀÏ¿ÊÎE?´¼ä@חž?ÀÏ¿ÊÎE?îÈc;í¯?œŽÆt?£yÌD±?œŽÆt?ïâKHËb?t3.k¦SÖ?m´·íÓ?t3.k¦SÖAGN4FGL J1830.7-1634¿ï«wœ¼LÀK~ƒ"×À8û6)‡¸ÇÀ;&‡¹E @P`@@̘å>³š?¸uË°4?ÍEɸÆ/¥@çtü+_)@Gx¶Ë¿Ä˜mŠ#!¿á*ÀH&¿ß'7<Ø"–¿ã‡ÄŸ×¡<¿é­Ìâh'¿ðUNASNone3FGL J1830.7-1630?æHa¯-»¶?È
þ«íN?Óo<¡¤ˆ"?È
þ«íN?åÐÆ+é?ÉIŒráì;?ÕÆ^s¨Ä/?ÉIŒráì;?ìœîÉTzß?¥ç—w'?»‰µ\)?¥ç—w'?ëfû¶‰a?˜äÝñª€0?Âd%Ûöz?˜äÝñª€0?¶bÕ@š?¸|ÍØéÐ9?í?3¥&ž-?¸|ÍØéÐ9?ÃÍ¥Øä?ÅM–ˆ3?ë?̾V‰Ç?ÅM–ˆ3?ÔÅöƒCZ·?ºguÏû?坾^R¤?ºguÏû?×Öb°K?±þ‹ž1Ãl?äÎ÷§õ[?±þ‹ž1ÃlMIXED4FGL J1830.7-3219¿½ÁJü:À$K-
$F0À:M)¹6íÓÀ;ï>FŒ¬K@
ovZzJ@òǝ¸ã?̱¬µÖB?КtŒB@K/©:÷M@]i·?ìŽPrß?ïùâå=¿å>f˜¿åOÍ2MZ&¿ë)˜JA¿ï…õåÊËUNASNone?ïã ^6ö?xn¹jF$:?lßü"ìR•?xn¹jF$:?ï§úk§ª?¤.²ë±0½?žkµú¦¹?¤.²ë±0½?îÀe¾JÓä?–3nn'û?£ù¤vÚÅ?–3nn'û?î'w‰(?‹/ÇYJ"?¦ØŽçm|?‹/ÇYJ"?§Ò'¼?"Ŧ§nûS?˜Ö4€ü?"Ŧ§nûS?è°ê|Ó ?Ìß@
ð?Í<V´±?Ìß@
ð?ëKÙ0C¥Ø?ªŸ'í3ô?ÂЛ>ñhŸ?ªŸ'í3ô?èsz}ib?·pÁñ§?Î2Š
Zw?·pÁñ§AGN4FGL J1830.8-3132¿ç×#/"ýÖÀ#aE•6À:>üGä› À<f°b2úÿ@ø$ EŲ?ýÖjÛ@-?Ãöó<?áwT€	û@0tBÇû­?÷ŒÈ¨zÝí?íÇh¿‡¿Úÿ'}ž;?Ç؎÷Õ:¿â,Æœ/¿ëº5¤¿ïý¾1)UNASNone3FGL J1830.8-3136?º½×š
æ?Äø°HtÛ?ì¿E¾C?Äø°HtÛ?Å|ƒªçA?Æ8F«¾'Ö?ê ÿßF0?Æ8F«¾'Ö?Êê?¾Ϙ?®<ïù¼]Ù?éEpx?®<ïù¼]Ù?»`(<gÂå?ŸÒÆû–R¬?ì"úøs£?ŸÒÆû–R¬?Ä¡äZ¡Ðä?Íc­Žîð¹?ê׆éW‹Ç?Íc­Žîð¹?Ÿ¢%őŽ?°_â?Ë_?ïîÑü®ß?°_â?Ë_?°E\ö¦?¢Š¾d?í÷T`æ…í?¢Š¾d?…\wë˜À?x|Õ³ç%Ñ?搜 6"É?x|Õ³ç%ÑPSR4FGL J1831.1-6503¿ïíȉµå™À6YTdÜ"«À:NRå€!ùÀ<‹Å£ãŸw@$Á'|D?ýŒMryš?Àúpßf,…?ÛRº·÷R²@RîcŠ	?üܼŸ‰?~@ÈG,¿•sG R›X¿Óðe£ráI¿ã˜a‹5S¿íçJýTT¿ïþ®û*®UNASNone3FGL J1831.6-6503?ªxrŠ9"ð?¸ÕšŒv?îXx×N¨Q?¸ÕšŒv?ØZ‹Jæ?Çý¶é[?ãÒºZŒñô?Çý¶é[?ÇÆídÇÕÂ?®,Õ!å?ü?êD¦Î
?®,Õ!å?ü?ßnŸß£®?³QZ<ÙÇ~?àH°1.)?³QZ<ÙÇ~?Ÿ#D7Cat?¹ØŒ,Ü?ïåÞ|Þ´?¹ØŒ,Ü?·xàÚ{O?¼ÑKÂ?íãä°2&?¼ÑKÂ?£D2bgy?–åÓv7©_?î˼Ú'.?–åÓv7©_?±Ï'àû›?šwô=?íÆ
£à"?šwô=PSR4FGL J1831.2+0202?à3eì*ê@¬óý">6À9ž;1.v5À;¡]³9@sŸ4
N@7ÜËè¡?Ê]u&Ê;?º;²!""?ïwLg·Ÿ@Ñ#rJö¿ÁŒˆy‹²%¿Ù'k\ÅRÛ¿ëÝQŸ"ë¿âKu°†E¿ä0#̎¿ì$P±*UNASNone?ïÖé6BÐ?{$Òр\"?t‹dÁ+t?{$Òр\"?ï]ä–åV©? S'Xš'_?"Cm!\è? S'Xš'_?î·~2¤±¿?™<šÊx?¤ˆÑia?™<šÊx?ïÀ'M¹¶?a´J~å?¶Ù4S©?a´J~å?î,5×8œ»?®ÿzá×?­<¢	éP?®ÿzá×?ëUðÿÔX?ÄÚ£º"ˬ?¨<®ž?ÄÚ£º"ˬ?ë¨1Kô'?°­žšÞˆÏ?Á_:Ð,õú?°­žšÞˆÏ?íIñ!Q?¡~ËXÐ?µ·Àvõw?¡~ËXÐAGN4FGL J1831.6-0223c¿îÛyaÚW@
orÖٖÀ8® HtäÀ:b4"F{å@~og–è@ñm*¥Åø?ÆèÐ#ˆã?ϏŠâq¤³@?òÿf}
?ù~‹=á7?ïh
?®–¬?ã"Ág	¿ã^PþJHN¿ævéki¦¿ê±ôÆ/¿ï÷™^á6çUNASNone3FGL J1831.7-0230?Ѧœå‡€?ÐZL¹"h?ç,±<z@?ÐZL¹"h?Ã
:Α?–ìãe?ë<±xL[½?–ìãe?ÚA&ç܃à?·þ‡î)‹?âßlŒ¾?·þ‡î)‹?Ë!Ws-t?­æaÞÂB°?é7ª8£4£?­æaÞÂB°? Çô³· ??¡âxñÞs ?îó€´à
Ü?¡âxñÞs ?"X?˜X5?¢‹dæ7?ïe>Í~Î?¢‹dæ7?ÄKšŒw‹ì?°Çs ?êí\â?°Çs ?ã¹['"?€C¹· ˜?ï‰øqÔò?€C¹· ˜ PSR4FGL J1832.4-0152c¿åý*Hð@
û–C£Ã¿À9*螺jÊÀ:ŸFŸ@èˆòWuÞ@ŽY½
·ê?Å};‡õ'?´Œ5'î²P?ñ³WN›o?í¹ž"!­?ïŸÈ‡Ã®@¿ã³Ú°¿åÓZ'És¿êYÙUm¿ØCÑ(l0¿îûž ç×UNASNone?î?n¸Íïë?»|˜0QÆ5?¬	wl"I?»|˜0QÆ5?â†a¹-ˆ¤?Î/Ûì>F?Úó<¤î·?Î/Ûì>F?éóüœHJ?±	ò›Ì k?È0
ŽÞՎ?±	ò›Ì k?é†ØÝã[Á?­æHú¾Ï=?É䜈rý?­æHú¾Ï=?êåŸp?ŅÆ='…ú?Äõ˸i'>?ŅÆ='…ú?»¥±p?ÅÞtªvá‰?ì‹^)ÎQÿ?ÅÞtªvá‰?éñVbžkø?´×S¸‰ªÖ?È:¦u†P"?´×S¸‰ªÖ?ÉOXdž*Á?·n9]6?é¬)ÎuP?·n9]6<MIXED4FGL J1834.2-0827c¿»ß׿²\›ao܇À88+"Ù@yÀ9­¢uá-­@'£Ýë-@D@yJ?È%µœ.ŸP?ãÖ³ «Ü'@[WG9?ô'qº,Œ%¿¸ºË,Ž©?áÌ•¶¿áP‡×Ð6¿í7åžTê¿èœåžªÐy¿ïõ'àhUNASNone?¸þŽVàÛ?ǙƒƒFŠÃ?ìà>îl¤?ǙƒƒFŠÃ? ˆF"û{,?£hþ	Dr,?î÷{—Ùƒ?£hþ	Dr,?ÒãóIZ´?²ErώÊ?æŽv[R¦?²ErώÊ?ˆ<ý @?tCóSƒ ?ïŸñ2»G?tCóSƒ ?¹™Þ…S]í?Мþ¼?ìÌÄ/U"B?Мþ¼?r†º»¼?sÃNÒS¨?ïÛÜòV@¡?sÃNÒS¨?džr«G?²öB_µ˜	?êcU9î8?²öB_µ˜	?ıü"F)?yœ¯‰ú?ïÿÚ9‹¬?yœ¯‰ú0PSR4FGL J1834.3+0613?ÚöÄË"@‰¼Ö_À:/ÞM'ÐÿÀ;èPÕ©³@,Eü
­@lKÅÑ0	?Ç·v¤L%?Ûê-/ãó@
Ew{a .?ù™²
ԚL¿äIq-iŖ¿ã»àÑn¿ßù;.ª¿â=@26ý¿ïúá¸\?Ôùr²¥ZUNASNone?ß6±o·^?ÌÄÀõå0,?àd§Hr¤Q?ÌÄÀõå0,?Õ %Ň^?ËP/d¾èÖ?åoí~<Q?ËP/d¾èÖ?æ½EÏÜ»q?±íJÿÑ´?҅t`F‰?±íJÿÑ´?åœ"[þ??°ñ‰Ûx›¤?ÕÄÆ×H'?°ñ‰Ûx›¤?¸äÖq6/?·šcÕ"Âß?ìã~%[Š?·šcÕ"Âß?™½UnC?¦ï(¼¯?ï2T·"¨?¦ï(¼¯?ËQœàuöý?¸á?˜Hã?é+˜Çâ'A?¸á?˜Hã?´b>¼f>?¡µw4ƒ¯?ís¾8_lø?¡µw4ƒ¯MIXED4FGL J1834.7-0724c?脈 x?Óñ(̧ãßÀ8Ní·þßoÀ9ógÁLf@CÏ*J+r@7õbLM?Æ('Á—å?Ýdéc±UM@_Ɨ(¦@I¯¡mÎ?ÖÔÀdïn¿Üœž^€>¿áWàÌV¿êÁ+Xô¿éûÔÂd"þ¿ïÿß~€8 UNASNone?ÊgÚ±ß-?Ï~­é÷nÑ?éf	Sˆ4º?Ï~­é÷nÑ?ªÔٖÌÅ?­€é¢Û­?îR²f¼nþ?­€é¢Û­?υš5mA™?²\½Ùàs­?è™r¤¯š?²\½Ùàs­?ºYp£oõö? »øÛqËâ?ì´Ñë'A? »øÛqËâ?²EÂ]ÜJ?Íw/+H?í½÷G}J·?Íw/+H?uÙÃü¸?"dÙ$±ø?ïÔMқÃÀ?"dÙ$±ø?¥½õrÍâ?›[ˆØOd?î¤ ©æÒ?›[ˆØOd?`÷U×`ñ%?RE^‡(z?ïï©ûD7?RE^‡(z0PSR4FGL J1834.9-0800?×{‡MšED¿‹ò7jzr7À8²ò03¤À9§†P¹Œ@diÁºŸú@ÿ³Ä¾
'?ÃʀÂ2??Ú)åè
@XÁTɅð?úS—™åô?ïtôhó¡¿Üá‡ÚTtÌ¿å÷aËÌó¿é¤cOοïýv:ÂÊ¿ïñ`[_wUNASNone?ÂàO^j¢?Ì"Š³;›?ëGì(eW{?Ì"Š³;›?¡ÛGQà?¤ºÖ'Wè?îïÒKor²?¤ºÖ'Wè?ÌQ£š¾ ¦?³Åõ½èˉ?èë—PwÖ?³Åõ½èˉ?'ȳ(!a?~4e]Šô2?ïi¿zúE?~4e]Šô2?µ×çKíØû?ÎeV
Ê?íE'Dá?ÎeV
Ê?rÂwBÞu6?'AËð/³?ïÚ{ª]?'AËð/³?¥Óí¿€†?™(û^Ì_?î¢Á/­8?™(û^Ì_?+°¦xâÑ|? Ûáå¯ñÎ?ïþDõ¹'B? Ûáå¯ñÎPSR4FGL J1834.9-2819?눣‡ÙþÀ"m‹`ñ²_À9ß)ã(XåÀ;¡?
×ÊW@A­RÞõ@õ†"X?ƃX$.]‹?Ì¿$³h£@©/¤2yÐ@jTXœÏ.?ï([žŒG¡¿äV¢¤W¿èû$Ų&¿ä¦^ê–¿ïþ×@Än?âÇÍSÛIgUNASNone?ï#ӈþ
?«Û"C?›†+Žà>U?«Û"C?ïB¤h2L?ž)Ti(Å?—«rô£?ž)Ti(Å?îÖ7"ð´¢?–šýÄÝ?¢œÏ<çÞ?–šýÄÝ?ï
RÜÏVó?€æPyè•Õ?žU¤lôY‹?€æPyè•Õ?ìƒÿ-ð?ºùô<K?»à^{…?ºùô<K?æ»+Áà=?Ï4Åb'ðè?҉©Æ|?…?Ï4Åb'ðè?èèƝ³¯š?²Ï~¡fY¶?Ì\å‰1A–?²Ï~¡fY¶?ç;1Á
¥?³ï˜–É·m?щœ}ñê¶?³ï˜–É·mAGN4FGL J1835.1-0517?Õ}5‹ä5…?óÄÀ:9tãë¸À;àæ½2%@¡ŸËŒÜ@N$PAa?ÔØèd?ïö?!}ÿ	@я1a@[î\>šE¿îäÍ_ê2?ï}ì?õ(?ØCôáé¿w¿éÍî \+z¿ìTÙÁQïa¿ï‹6môOUNASNone?ԙsD¬h?ÊÌÙµÆÿa?å³F]©Ë¸?ÊÌÙµÆÿa?Äh:ËqDz?Ã4Þ¢ðÛ?êåñM#Ž?Ã4Þ¢ðÛ?ã‹Íu‹"Á?´.1c‰Ä
?ØèeèÖ?´.1c‰Ä
?Ȁ1ãÓ@?¯ïþ'©5p?éßó‡:‹0?¯ïþ'©5p?œ8ZLm:?¤ë­0€?ï=-eœp?¤ë­0€?'hÔôœF3?žDNJa¦
?ït¹X"Y?žDNJa¦
?ÁQA'£Ó?°#)3ˆ¡?뫯Ÿ{—?°#)3ˆ¡?œŽœ¯[t[?áŽÕ®8?ï‹i§}?áŽÕ®8MIXED4FGL J1835.3-2439¿îaR;ÚÜÀµK 'ßÀ9¿WeA£8À;]Û8 Z~@2۞ ç×@‹@š?Ä2·¸=Ÿ?®h²ñÚMi?êHQY•?ýŽücé4?ïñ"aÔ±H¿çMž§öT¿ër4€:M¿àõÓ÷cyL¿êm)™V}»¿ÛVÂd>UNASNone?ï">þ?­‡é
XÔ?Šúp2½Ît?­‡é
XÔ?ï›+Xã
?©‡(ÌԎË?žìšŽfÌ?©‡(ÌԎË?î±úpko\?—Kkƒô¦7?¤àXôý‡D?—Kkƒô¦7?îò%'>d?'YH€(W®? Ý¦Üõ¥8?'YH€(W®?ì¥ÃlC?¹`ýû"À¯?ºÑ䛗íê?¹`ýû"À¯?èX³Þœá€?ÌqÎ@À:?Ν0…Œyÿ?ÌqÎ@À:?ìg^`*¬?§ÐgRá?¼Åþ¯â ?§ÐgRá?æý{64Íñ?²€]#'Í6?Ò	"–d?²€]#'Í6AGN4FGL J1836.8-2354¿ëè×'™¢À"?ãDÞVÀ:BžHUÀ;¯ô"q<@
BTä2ð@ä¼B;
ó?Çè-%}$?Þç	úTÅT@*ܾ²W×@ôòÌæ£
?î)Xb—¥¿Ù¤›À»F"¿à]/…ÿ‰¿éÅ>=}d¿ïúȈšmÕ¿ïü™^
wRUNASNone3FGL J1837.3-2403?áX»zagp?Ëës÷"Ã?ÝN‰=1?Ëës÷"Ã?ÙPAÅáåÒ?Ë4P¶YT?ãWß
?Ë4P¶YT?ä'‡J©‹?³‰¹¢£'?×°ñ×j¬é?³‰¹¢£'?â›t}Ü?®L¡áj'a?ÚÉýÑH?®L¡áj'a?¸éÏ<€ÉE?¶c­S£?ìâÆ}¥G?¶c­S£?ª²çQìˆ?µeæúñ?îTъîþG?µeæúñ?¹ùï–a'ü?§$­d֝?ìÀÂ
3ÍÀ?§$­d֝?µ¬h€iiH?œ°&hò?íJrﮧ?œ°&hòMIXED4FGL J1836.9+4439¿Ûå Ë3'õ@5!S‰Ò|À;
»DåÀ<Ì&Tþ_@ ìw‹§¾u?ý7†ª×¯?ÒQ/|}?Í|õžþ'?ö5…£BÈ@AÊ¢ûíø?ïÿn?x»Ô¿ïÿ"~LŒ ?ïó˧nn¿âº‰ yÞ¿ß:i]f¸q¿ÖÏo~èé8UNASNone?ïùåZsz1?@¤ò5
§?Hj• gË`?@¤ò5
§?ï붢—?iª¡¬s&?dIâZ©Gû?iª¡¬s&?ïÕ9ýÊ*?q¬Ñúàd?uc7#¶ö?q¬Ñúàd?ïÇ枅Ë?eVg0?|°Ç'3?eVg0?ïù0'1"š?L•²<ÔJÞ?K?d	|]g?L•²<ÔJÞ?ï§ZN?jHŽ³8?†)y6|ݯ?jHŽ³8?ï¡r_—Ñ?†_‹ ~?‡£`.ùC¢?†_‹ ~?ïsxŠÖ2Q?"¡#éڞ?'î£çÜ?"¡#éڞAGN4FGL J1837.9-0620?ê,L>œóÁ?¸Þm^'RªÀ8œá8"œÀ9ÔQžXE@äq–ñº@…à1?Ím6d@y?Ò¹–å	Y›@Ùs¤<ŠË@#ûó+g¿éMóÉøÝ?Ùä¼Îa¿åvÿ:Þ"`¿Ö=9T¿ëÍ/(·Ä¿ä?©þk«UNASNone?á…Y"­?Ó×íšÖ89?ÜõÕLÖ¥ò?Ó×íšÖ89?Ê(>d·3?ÇÉD¤l'é?éuðfÒ>s?ÇÉD¤l'é?Ø0¤i¢¦?µ¯C¦¨3?ãç­Ëw.­?µ¯C¦¨3?áרÕÄ°?¹X°ê²Õš?ÜP®Twâ¡?¹X°ê²Õš?ËßLÏä?яpا˜Ø?é,þLû?яpا˜Ø?'Úx*4ç%?¢Õ¢lþQ?ïi,>w_?¢Õ¢lþQ?ËÔs	aþx?°Í,þڞÄ?é
ã=§€b?°Í,þڞÄ?£LR7ó?™å<GQ?î΋>ôÑ?™å<GQMIXED4FGL J1838.1-3352?ão4òbÀ(f¨ü
,8À:·?Úáb†À<˜úà@*¬C•V@茊½^?ÔzD¿¢˜?×c0œ*¬@|íáðJ€@u+ùX?ïÿÏ"èbU¿êƒÙ©T!À¿ÛÆ\Õn¿æÈl뻥]¿çžôí}F}¿ïü¥'†·UNASNone?ïQsCÞ@?¸Å¶{ˆü?•Ñ—‡§›é?¸Å¶{ˆü?ïB%ÇîIR? ² ,¨üú?—»G
ÍÛ¸? ² ,¨üú?îRÊìçŽ3?›rXv´sW?ªÓQ3>êÎ?›rXv´sW?ï[/.Ir?€F•݃?Ÿ"š"Í×±?€F•݃?ïÒÿGY—?ˆý²ó²¿°?v€\?FÀò?ˆý²ó²¿°?èÜ®¦¾g§?ÊóÎÏŒ1?̍Eeae?ÊóÎÏŒ1?ìI¢¸ý0?ª^ê'?½²ê8ž'?ª^ê'?éØo]Ù?®÷³âÓÇ?ȟ¶B‹"?®÷³âÓÇAGN4FGL J1838.2+3223?'¿d¨wã#@0´£ø˜,²À::Å%8ž­À<Ñ%÷áN@°ZŒ¾iÞ@^P?³t6?Åòw×'É?Ðÿ ß‰@ºVwÜ?üºËÃbk¿áòýž%ðU¿Ñ	£ðÝM¿â͇<ŸÃ¿ê7‡UÊ6ð¿é5:ßÏÞпïÿöùŠpUNASNone?ï2II±5(?¢'µBî?™¶Öˑ)?¢'µBî?ëé<×Ì°?¾§`…뀱?À[ Í?Ž?¾§`…뀱?î•	žÜ›ï?—¡\ÚÂý?¦¯f~s?—¡\ÚÂý?ìY'K$I?šÐâ#=u?¿}3m¦Ý¶?šÐâ#=u?âàœ38!ì?Ç÷Ÿx°ð?Ú>Ǚ¼)?Ç÷Ÿx°ð?Ú%à¦ë´?Ðì	ª	®?âí¬Š%ø?Ðì	ª	®?ä(ñMhF?¹ò/,­Ä?×®äe/s?¹ò/,­Ä?Ö#ê0ñöŽ?³B5"¤{å?äî
燹?³B5"¤{åMIXED4FGL J1838.4-0630c?ëΐ=Ç®!¿¶5U"…XÀ8ÖòJ¶ÝÀ9ßL¤@!7væfPí@ÙÒmrÊ?âh°ºG?¶'à~ÀÃ?òÈ4L7æ÷@—IEbø?æí½¨l›4¿ë,$ˆþA¿â*Œ 	_пéÇô@.C_¿êf££׿©½ï¦ìhUNASNone?Ü£¡îŸ'?Ôz%D€?á®q¯°m?Ôz%D€?êÃÑdûÆú?ǝ`²ŒŸ?Äðºlä?ǝ`²ŒŸ?ázè§Qp¿?· "o'&³?Ý
.±]ƒ?· "o'&³?í%û|/ð?¤.^¶dn?¶Ð$$ý?¤.^¶dn?ÐÈ_ðcç?Ól¤JÖ?ç›Ð7‡Î
?Ól¤JÖ?Ýü÷Ýqµ¥?Ô â¹Å€?á"G%.?Ô â¹Å€?ãoÍh†¯»?»"Yqi?Ù e.ò ‹?»"Yqi?Ø´Ž°±?ÆýlŸ2?㥸þ'§~?ÆýlŸ28MIXED4FGL J1838.4-0545?פ¦YÞ]?Ïþçüþî³À8Pª<À9LWšÈÙ@#ì°	‡@1ó:ß¿?͖9'ÈÅ?Ù²…"êÔ@<¬Ñ"Âr?ôªm9>e?ƦÊYªì'¿ÓÁ*¡OÆ¿ä€þ "o¿ç¸ˆb½Þ¿îxIRYi(¿ïä$7í'UNASNone?µÇ3"|à?Äú¹ãÇ*?í_‡dU?Äú¹ãÇ*?¦ûZ)ÇB­?«.^¯…5¬?îJ]qJE?«.^¯…5¬?ÐøEr69‰?³«n¢$L?çƒÝFäã;?³«n¢$L? øh¦Ålª?‹ð㲋eÌ?îðyujmæ?‹ð㲋eÌ?¿Ì¯¬¼;?Ðà Jžñ?ìj
hlY?Ðà Jžñ?v-{ÂÒЭ?‡£l7?ïÓ¥˜/?‡£l7?­Å†j9?›‡Ø^Í×?î(ãpŸ?›‡Ø^Í×?:•MŒq?0^\'Éc?ïü­V .Z?0^\'ÉcPSR4FGL J1838.5+3837¿ÂÔ
­V~¬@2áô™=SÀ:µÌ÷"÷sÀ<[]À¥w@"?6¡§°@Æñ'9y?ņ¢Ücm¹?ƒd·î!
õ?¼öxýí@õýÁ¿Îeô{'r‰¿ë]BÑ5è¿ãù½@gÏ¿â?õž}.)¿ïý'ÞZ"¿ê;Ì^èãUNASNone3FGL J1838.1+3827?ïón³M0?QÞÝ%¡ƒ€?Y"™` j›?QÞÝ%¡ƒ€?ïëߞã¨?l愢à??d<`¥Ô‡Ï?l愢à??ï±Ú,?€`:‡?ƒ¸É"sº³?€`:‡?ïãïML±V?Tª‹g?l²ž±,?Tª‹g?ïÍ÷Ì¢&þ?x`Ë)Y»?y¥M˜î?x`Ë)Y»?ï¥hbr™ƒ?8îÿ•?†¥çt‡«?8îÿ•?ï—¹®·ä?‰óËèkü¸?Š8âk?‰óËèkü¸?ï\,üYÅ?ÙÉAç?"z`nTÇX?ÙÉAçAGN4FGL J1838.7-0601?áL8±–?°uÙöÖáyÀ8öþ	…»À9ýtšÜ¸@"Ž3ºí|E@ir¥9

?ÏufI
5
?µú¥D"?ðŠ"˜±<N@֛öEŒ¿Ý(âø2V¿ÀQ°â5"·?ͳb(¤9¿ß¼¤`œøÊ¿æ{ï?z¿á©ø!mUNASNone?åËt+1BS?Ò'à6-†?Ôi©{Y?Ò'à6-†?í;N_ïÌ?½vuäCó?¶%4$š ?½vuäCó?ãòݐœùS?ºâ—Î?ØDÞÆ
Z?ºâ—Î?îwÕ¤? 	(‰Sm?¯ŽH€íé7? 	(‰Sm?ä xƒIv?ÐÊì_0´u?׿ùmÕ?ÐÊì_0´u?æªX0v?Ðxœ#a®ò?Ò«ýOݟ?Ðxœ#a®ò?ä=œ0€Y	?Ã~Ž®â‰«?ׄǞÿMí?Ã~Ž®â‰«?刭+ØÝ
?Âf6ø‡=?ÔNEç?Âf6ø‡=AGN4FGL J1839.0-1502?èø×0˜À‡zA¾	À9–ä+Ž#À;4Á5¿Õ@Ÿ?´öÂ?@›:Æ¥k_?ÉCáè<ë?ÓKaþ!Ùo@ÊôW@eÜRÑ´?ïÿHë+\¥¿Ý2/'"š¿é(¯ Ä¿â7wÀÖÊR¿ï®+ALP'¿ïÿø]ˆòUNASNone?î"E¢Õ
<?¥GJá"?¦Ë¥ÑÓuG?¥GJá"?ëîˆëK+?¼Í#&ÿ%î?ÀEÜQ¾ÓT?¼Í#&ÿ%î?ëËù2†?¦êzk¬ò?ÀÓ¼4õç?¦êzk¬ò?ì \«@yÜ?˜˜ÙÖ[?ºý¥ü1?˜˜ÙÖ[?æ7Öï̒Q?Ê*íòêÌ?ӐR fÛ_?Ê*íòêÌ?Þ֛?–«?Ñ!ŒmÈ@²?à"²`~´«?Ñ!ŒmÈ@²?âŒÏh!kN?·~l{*"%?Úæa/½)c?·~l{*"%?ßXHM?¶"Ò×x®Z?àS¿yõ[Ú?¶"Ò×x®ZMIXED4FGL J1840.4-1705¿ç±€x‹WÀ]^^Z(kÀ:NH;Øô"À;¸©Þ‹;2@ ‰iw½Ñ²@½D™?ÒYª–A ?Ì'—ÉŠÍú?üö¡ÍDÁÑ@xœHöi?ïíTa$X¿îL'\f2?Ùþb;^zà¿å°ý-½¨m¿ìêÛ@-¹?Ä=må™!UNASNone?î·óؐ‹?¡oQ•Á??¤€Â{BÊ?¡oQ•Á??î?ü6ò°a?³«Ì/şÅ?¬<'ŒÇë?³«Ì/şÅ?í–õ!ՒÄ? ýús!€p?³HVðåv`? ýús!€p?íHP¼0}?žYýB"žÂ?µ½zí"?žYýB"žÂ?蜕¨Põ?ÂK†ø=z?͍©^¼+?ÂK†ø=z?ç|æؼš%?Î[…	È3i?Ñ2N†Ë·?Î[…	È3i?æÀ"ÂPXC?·ó̉é ?Ò~Ø{_Oy?·ó̉é ?ã:~šÔpõ?¾jq^£4´?ًÊW?¾jq^£4´AGN4FGL J1840.4-1139¿èà½F¿NÀlÀóz¶À:™[†8"À;ø÷§kê4@ËK;½›W@'Wɱh?͝Çüƒs½?ëkö}ö%@œ(²¦°Ù?þ8›7(‹:¿ïým´8Q?ïÿñ¢o+1?ÝKáÕÈt¿çW½@½µX¿í¬¾¿ÃÏοïµ{A¿½ñUNASNone?º'¾´Uª?»ÜiÖfM?ì­¨)UK?»ÜiÖfM?²~ÞD=æ?µÆ€'';?í°$<<ó?µÆ€'';?Ólb¥wÚh?±R=Âö?æIέDÌ?±R=Âö?­r©Ê!r?'å+G¿LÖ?î(Õck¬™?'å+G¿LÖ?nNfÄÍ?'¡çºÇŽ5?ïár±ÖÚË?'¡çºÇŽ5?€M˜óÖß?Šo2>(¿?ï¾É~'½?Šo2>(¿?²Že'íƒò?¡o×y/3"?í®3OkUÂ?¡o×y/3"?p©øO"@?c."Ñ'ê?ïÞ¬_eä?c."Ñ'êPSR4FGL J1841.6+7113?ɺ®š»5@:Z–=Ć­À;tµcú{\À<ö«Yµ}ü@ ךÊF4Ã?ÿ׉¤Y=?Â$$wƒš)¿©CH ¢"F?ççf¬ƒ¨?ÿ¸Bi\ ¿ïìÎ?=­‹?ïüZžÜúl¿ç÷>Ælª¿ÊkÒ6?è¿à@H»ÊF¿æ&ÙRíÞUNASNone?ïý½èO×{?$,Ç2?2½Ü†"^?$,Ç2?ïïJlo?bL°ß?`µ"ÿ™?bL°ß?ïñ¢Š#¡?\^d¡)¯Ì?\ºìTnm¤?\^d¡)¯Ì?ïèŒu¼5?NòÈ\ݍh?gsŠ0°úò?NòÈ\ݍh?ïüZ˜õ&U?9vDœ¸?=+:\¬Ì?9vDœ¸?﮽t.þ?'
Mövø?"P¢ïS–r?'
Mövø?ïòJ¦¤?iVÞ
CD2?[j´/Æ6ô?iVÞ
CD2?ïp®t$ȕ?ƒÍ8¹<ü?'ê1{fíd?ƒÍ8¹<üAGN4FGL J1842.1+2737?ì[‹cmZ@,+ææS†À:K½R†À<ˆd•y@Èü¶õJ?ü…Ö|?Ķ"‹ë[-?ä†ü^	öy@eê«%)@ÔCíë€l?æÀv蔩p¿¾z% x…ù¿©½XÚ©¿â§ÿ¸ÝW¿î͐ ôí'¿ïžÏÎß̄UNASNone3FGL J1842.2+2742?Ò|Y[…?Τ2ÚrÒ°?æÿAÓxÒ>?Τ2ÚrÒ°?ÆýˆK¾og?Âd<µ½ç'?ê@íd&?Âd<µ½ç'?ԘÞô½²?²®|džrï?峐…ô¡'?²®|džrï?Õbd}q߅?±-Kâˆt#?åNÍÁG=?±-Kâˆt#?¼Ôd=8½?Ȏ¶bc]¯?ìesxXè`?Ȏ¶bc]¯? *Þp¦?Ì?¨¢²<Àµ?îýRÚ#?¨¢²<Àµ?Á)¾oç«?¯à«q eÂ?뵐~¤?¯à«q eÂ?©3"Í;[?–Æ ö ©Û?îlÇ-ügš?–Æ ö ©ÛPSR4FGL J1842.2-0328¿ëïäŒå‰»?Ý:
b>8 À8hÞ4Ô#À9¨XŠÑ @Å÷ùñÉ@Òa¤_Æ9?õ¥ouÙ ñ?Émµ$ºt†@5%1?ûrEî¿ìxÄ'6N?íÿ*¿åc'K¯¿ì'<ðKW¿ä • ãû=¿ïÿÿÊPËUNASNone?Ý[ ?ÄÒ?×+ßX7?áRoàó—?×+ßX7?ÐÿŽžœk?Í1ÜYW›?çô€8°±Ê?Í1ÜYW›?ÙÕ	–E–?µÄ±_pïP?ãu{4Ý5?µÄ±_pïP?àiß0–d ?ÂV+ûÜYÞ?ß,AžÓ6Á?ÂV+ûÜYÞ?Øøo§IÓ?Øס	®B?ãƒÈ8,[?Øס	®B? 3˜î)è?±áx•ù?îÿ¼ÆšX±?±áx•ù?ÖѮЯÓ?ºs5µL08?ä—v¨—¨?ºs5µL08?šÈŽøÌr?Ÿ›î]–3?ï)»ˆ+Ýÿ?Ÿ›î]–3MIXED4FGL J1843.3-1242¿Ñ¢çöô¿ÀÿdIU´gÀ9Ñ{m^¨,À;pSÒ+í@Ž•¯4@£þwiÄ?Ì¨¯â?ÒåAbËÒ@'ö¿ž(@#V/ŒŠ'?ï;Eñ{ؾ?î/¥>éIÛ¿á<DSìç¿å«LŸjéٿ퐩e¿wz¿âÜþ=ˆ ËUNASNone?îà(òg'	? d'ð$Ž×?¡ýpÚbÖr? d'ð$Ž×?é.	–_[
?Äóó	2Ñ?ËGÙ¦'"Ì?Äóó	2Ñ?ëc±v–F?¨®ô)-?Âsñ:%¦ê?¨®ô)-?ëòVãLÒ'?ŸpÌD¾U?À6¤rÌ·d?ŸpÌD¾U?ãB!ׯî‰?ÉÕ.6/x$?Ù{¼P "í?ÉÕ.6/x$?Ø:ïÄb^ß?Ò* DØ?ãâˆÎБ?Ò* DØ?âp¹åÙ'?·>ê8§î?ÛŒ4M±Ü?·>ê8§î?Ý>¦ˆ.Q?¿À›!j?á`¬»è×x?¿À›!jMIXED4FGL J1843.7-0326¿èÕʱ¶?¹hšY³À8/r&À9|_æ¤í@W­»åt@ºd<Àz¯?欂ªiËv?¾²pK˜?ûV'QúŸ?ð•˜/âè¿mÜ	‰IGû¿Í—Ðk½¾<¿äÉh^Ž*Ñ¿éªÃø贊¿íþVèD!˜?ÜõÇb)ÀÄUNASNone3FGL J1843.7-0322?Óˊ=Â>?Õ×ÑÁ0ë?æ:áà¸?Õ×ÑÁ0ë?ÐùÓÙ?ÌôÇ+'íí?çƒ|–uð?ÌôÇ+'íí?ÛäòÇÌ÷"?¶Ðbîº?â
†œ">?¶Ðbîº?Ûj""B[U?»)ÒGœ2?âJ¶nÞÒU?»)ÒGœ2?Ø!y}x?Ø-K…ä?ãðowÃAD?Ø-K…ä?"";•l?¤‹YÌ
kO?ïca'óæu?¤‹YÌ
kO?Ù-¤þ҃?¿–ÀÕD?ãwé-€–¾?¿–ÀÕD?'Ê+ëgØÜ?ˆKšM­D?ïi® Íü‰?ˆKšM­DPSR4FGL J1844.7-2110?édg
{.À +éȆ/À:Wꢠ©À;³§¬_o@W欜֐@Ov¼Ï)?ÊY&âÂØW?ÌÒ÷_Ÿù?ÿ'zH›zD@0‹1vðw¿×7¡2À?ïû@>Æå¿ç¦âøˆ<z¿â¯Dü‰Rú¿êàx`cíæ¿ï÷#b…±/UNASNone?ïr&ÆñÊ?¢« nô§?'»'ç†
?¢« nô§?ï¿Ðîx!?¤×ÉüŸ«?Ÿˆày-è?¤×ÉüŸ«?îî"2yƒ?"[ò	}œ?¡ÜÖL€Ì?"[ò	}œ?ï'Ôú\–É?}$íz[!?›`»L^ã?}$íz[!?ìy»ŠA¸?¸S]ÎÍ?¼2#"­òA?¸S]ÎÍ?ê5DÃ(‰6?È4KŒ€	?Ç*ìó]Û(?È4KŒ€	?èr‹Z3?³ú¼¦èKS?Ïþ5җ3…?³ú¼¦èKS?ê@Ã("!Ø?²%?	î$è?Æüó_wx¡?²%?	î$èAGN4FGL J1844.8-0957¿ÏIµ%TVÀ‡«¨À9€_7ûÿÀ;Íì‡}7@Á¡w‰yf@Ö$o…Ê?ÌY{ÜÅ=a?Ôn›¿
Çi@tòñ#Ä*@¦Ý>ßå?ïæÍ)Á¿ÞôC~"ë7¿ácÍ.ò\¿éÐÚB×%¿ã#¡?€H¿ïü¯ž=Ã/UNASNone?îú©aì6Ó? •³Ô)ù©? UiâyÏ? •³Ô)ù©?éVæEµÆ?Ã1štéi™?ʤfëá(é?Ã1štéi™?ë¬ãLYä'?©Å>7Yo?ÁLrΘm¹?©Å>7Yo?ì,»ŸÓÅd?šžËšŽ/Z?¾š#aÔÜ?šžËšŽ/Z?èUérŽ¬š?ÂHïˆ
«?ΨZ5ÅM–?ÂHïˆ
«?ÒÀ.­¬9ô?Ïø©œÎ?æŸè©)ã?Ïø©œÎ?äè‰|ý?·Lªà`Iä?×.íÜ?·Lªà`Iä?Ù Cè3õ?· 
JQt÷?ã/Þ7‹æ?· 
JQt÷MIXED4FGL J1845.0+0159¿êÝТ'²<@¡®ÁIÀ:Œ°càz)À<:.›ô½­@žªÂ`ã?÷}}8Ð+?ÑüU›½á"?ïÿ?`h¤@¤Æ†"Ä?ûïm£Çoì?é|Ÿ5åÀ¿ïø''ì×.?ïÙ8`C·¿Üê_d"(¿ïþß~«+½?ï 'àðUNASNone?Ù&Ÿr\Ïö?Ða‰&ºÀ?ãl°Fј?Ða‰&ºÀ?Üq£~ÓMM?Ó¤¹Íš?áÇ.@–YY?Ó¤¹Íš?åLTh¯?²¢¢¡µ?ÕgÄáW.¡?²¢¢¡µ?ށÑMú›?¿u þÓ/=?à¿qÙ³?¿u þÓ/=?Ò«riÔÚã?Îào-¬­ë?æªFË'Ž?Îào-¬­ë?´=Ó!?ÃÁÀeq…?í}½87Ýp?ÃÁÀeq…?ڈo£"‡—?´¡ÖHvm?â»È.=¼4?´¡ÖHvm?ÌâãU‹ˆñ?ÁöÚfiä?èÇG*Ä?ÁöÚfiäMIXED4FGL J1845.8-2521¿ïܲMùÔÀ$=:uFÔÀ9"Bþ'Q~À;Ì"ð½m@Sj¯÷)@DàÑ?º×ý­j[é?҂A©¨…@Í%îÇÉ?ô@gÌm‰?ïðcu^P¿àšdÃÎ÷¿ßn{=Ž¿â"º?+Žú¿ïšˆ!L*ü¿ï›¡æoUNASNone3FGL J1845.5-2524?ÃÔÛÉא?ÃYžjAoê?ë
É
¿J?ÃYžjAoê?ÆÙš%I?Æ+p̓½ ?êI»Yv­ ?Æ+p̓½ ?ÚÃ#÷è¸?³±Ê¤êµµ?âžnõ¤?³±Ê¤êµµ?ÄÜÊj`µ¼?¤åEºUn?êÈÍegґ?¤åEºUn?‹ò˜¼¹?©»©°ZSÈ?ï5Øs?©»©°ZSÈ? œ‰
3?®ìµ%ŠTâ?îþV7¢·-?®ìµ%ŠTâ?­Vù(MæŽ? o¢ÞÄ?î*m²W? o¢ÞÄ?†…MDFû?tõï]ï>?隣êô*4?tõï]ï>PSR4FGL J1846.0+0507?åÿ!5"Ç%@HüBÜ£À:8ÓMŽÀ<Æ
:ìe@fþ¥7§?ûIR>'5G?Ì5?ÒÓÍ?ã'-Ê=¦T@°—"ìck@`{—%  ?îž›aö¿ì´=õ.æ?Ã:öËù¾¿ÖÿÊ{
èK¿î'Ó¹PF¿âúy]¹ïzUNASNone?ì@ŒyÂÜ?º2iÔ$?½ûœ1é ?º2iÔ$?èMé!þ?Èÿ5•85ü?ÎÉô[x?Èÿ5•85ü?ê1tíç?¬£Éækîá?Çã:,K¸e?¬£Éækîá?複®W
O?­2 nÓ{?ÍmáF£ÊÂ?­2 nÓ{?áãh•@?ʂrb.Z?Ü8áù.Հ?ʂrb.Z?Õ­ê!?ёŸÙ¾fœ?å)
øxïw?ёŸÙ¾fœ?ãYÎí°¿r?¸]kŽ8?ÙLb$ž?¸]kŽ8?ÞHWïÍz>?¾R	.ŸG%?àÛÔBá?¾R	.ŸG%MIXED4FGL J1846.9-0247c?µ 7ÿ†ï"¿Ñ÷u¢™r'À8Ž€µÀ9þ±¨ó@ Ë´Hòb@? äçuÅ?ÊӚFgÃ^?Ú1à!é3á@LfÓs¯û@
5^†ž¿ã€¿ð©K?í§\€3—¿âp*ՖŸê¿égDýàëé¿ïþ Eð¥?ïiQ;UNASNone2FGL J1847.2-0236?åÛ,¤ê¨?Óûm³{†Î?ÔI§Ú¶*°?Óûm³{†Î?ÈEÙéjè+?Ç>9«-§?é¥Eõ?Ç>9«-§?Û©²bà—?¸yd
!´3?âu«&Ώ´?¸yd
!´3?ß|¶uaE?¹
?Ô¬?9?àA÷¤ÅO^?¹
?Ô¬?9?È$ ùo?Ñ­U–½û?éöùûÁ¤?Ñ­U–½û?†¤ñì?"}uDÒ?ï§ÝlWA/?"}uDÒ?´¥êZ³G?¢k«áÏü?í~kB™,·?¢k«áÏü?—ˆ&†zΕ?Ó7FÓ?ïC¾Ì#K?Ó7FÓ8MIXED4FGL J1847.0-0625¿ñ""(–D¿ÿ-O#SÂÀ:GwÀ*ýÛÀ;Õ+y*ŽI@k÷τâþ@eXê|àü?ÏÈ÷ê‡É?àþ_o×(@¨¯bk/@Æi/œY¿ïýêªr/?ï¿©~+V¿ÏåH U5¿Û¯Cdƒ¸1¿ïiÿºùf?·Qx!$UNASNone?í'?YvÔ?Å҈è5LØ?³n2˜#e?Å҈è5LØ?é 1
0|í?dž³VØÚ?Ë;×>M?dž³VØÚ?ê/ñ0žO?«ÔÇOæ|?Ç@;=‡ŽÄ?«ÔÇOæ|?í[§ŸÛkæ?•uMõË!?µ"ö­R?•uMõË!?æ «"Fë'?ÉÅĜôå<?Ó¾©»r(ß?ÉÅĜôå<?Ó«ӁX?ÐõCYØÌ?æ*r?Sõ?ÐõCYØÌ?á WLSPñ?¼|Eãö?Ý¿QgY^?¼|Eãö?âo0X´'?½{£åLöS?Û!ŸOĖü?½{£åLöSMIXED4FGL J1847.2-0141?ìŽÔá0:?Ē®Bóð}À7å·lé7À9|¡|¼ê@Œè¹èC¡@ #¦Î5ƒ?Á!¯}0­G?Ö92¼î¥@}¶åû@f·Œž´a?±öí ™¿½?¦´	\u¿á ÔV.	ÿ¿é&Ébµþ¿î"]à…ç5¿ï¥íš¢®UNASNone? FDhÇ?¸h÷˜Ûâ?îû›¾{À?¸h÷˜Ûâ?¥"Ï͋£2?§¡åÑ':Ý?^??§¡åÑ':Ý?Á'~ý"žf?­€Ë¥,
O?ë¶ @šØg?­€Ë¥,
O?¯ Tw:D?š(m ÛÖ?îú¸ÃU€?š(m ÛÖ?¤vè«?Æ:SÙÏ?žÊ…ö?Æ:SÙÏ?t¡4Lí•?'ÀöŽìß=?ïÖ½—áĽ?'ÀöŽìß=?³ˆÉ‹Ñd?gÆO:"?ï‰1ܾSÛ?gÆO:"?IìYçÕ?@´qDAQz?ïù"þNqu?@´qDAQzPSR4FGL J1847.2-0200c?çf¥v»?Z8ž'6§À8`§GØæÀ9³a°ôÿò@ †l(T@å eÑ1?Û'¾Anµ?ä'ô>UÑ@ŠÎ$»¡+@›¶‹lÛ ?í")à¤&¿ãւN8ó¿æ›»øi3¿è$nß±«ß¿êLÆ¢fFÜ¿Úöüᒁ¢UNASNone?äH|:Z'=?ÔX)z€W\?×o‹J݅?ÔX)z€W\?Ù ÎÕn9¢?Ò,ûU÷-t?ã/˜•Hã/?Ò,ûU÷-t?ÞëÌ03"?¶Ô,1t1Ï?àþ
çæ6?¶Ô,1t1Ï?ׯɺQR·?»ÎK§ô%V?ä("×V¥?»ÎK§ô%V?àþdA!'?Ô~rhz×?Þ6Å}¼Þ?Ô~rhz×?µ…'
Ÿ¯ø?ÂA—ða?íO[¬
?ÂA—ða?ÓýWµ"ÂÙ?¹³žä˜Vµ?æT%=ž"?¹³žä˜Vµ?—'èñÏ?jP`'£?ïCh¸®»G?jP`'£<MIXED4FGL J1847.7-0125?ï}¤#=ûA?ła€"¥À9PþöÅÀ:z¶ƒn@!ê
¬»à@@Ca~ ?Ï<â()?¸.žp?ïÍ4›èÿ2?û;Tiä ?¯òlÄyl(¿Ú|#¼ó'¿âð|iÝê,¿êSb}¤¿àµfÿ"s¿ß½×üÖªÇUNASNone?èúƒ*p?ϊ"ºÑ3?ÌóßW¶B?ϊ"ºÑ3?ê¾/Ïë)?Æ+fUt{¨?Å@ÀS[Œ?Æ+fUt{¨?äa°ëV?·ôÀ¡Ç×?×<ž)Séë?·ôÀ¡Ç×?íßX·ôp?¡
š9†ò>?³';C?¡
š9†ò>?äuðÕôy?Р~À'ð?×TÉ?Р~À'ð?Üt'É›¿å?Ôµú€í¯?áŶ›2 ?Ôµú€í¯?ä8ùmŒò?Âʗ%ԃƒ?׎
$çÒ?Âʗ%ԃƒ?ÞrÿÀ®Ë?Äû7IÔp–?àüF€¨š?Äû7IÔp–MIXED4FGL J1847.7+3543¿èEéUˆ#@0!†¹ÃÍÀ;Ÿ¼
éÿÀ<Ͻ¥œà@!j\‹ò?ñ•:uFÔ?ÞÆÀQ>a?ì¯:€.Ž‰@P¾yLòø@Ú%ñ]É?ésÌ`@\'¿ð?í—ß…65?ïÿû˜'2¿ÞÀÝ`í²¿ïþâ~dßÔUNASNone?ïë65W`ö?_:÷:E3ƒ?dÉ'¼?_:÷:E3ƒ?äe?Ÿ1®AÕ	?‰×[Êj£?Ÿ1®AÕ	?ïmXQ6?‰t")MŠ?'LTùHÚ#?‰t")MŠ?ïH rJº?‰Ñ»ZDÖ/?–ûü)¢Ì?‰Ñ»ZDÖ/?ïÆ`ÒRÈ¥?H!êþì{?|ϖô(Qr?H!êþì{?î›ÿõe"§?¶²¶
Hâ?¦@¦7™?¶²¶
Hâ?ïötL>X?™0ãa^ ¼?ž1{Ÿžñ?™0ãa^ ¼?îíq¶·ÈÀ? ýhËñ[?¡(ä•_[? ýhËñ[AGN4FGL J1847.7-3433?ÜyDW¦b³À,˜â~ù˜À;<Ž%ÈÀ<£yv
£W@‰nMægÓ@.Qúž—/?Ïê¯ iú?àh…à19@MZ%æC–@L¡°ƒ•?ïûñ}†=œ?ß8KgÝ_¿ÑúÍ%¸ m¿ã˜àkæ(¿ïìÇÿ]˜·¿ïÿàöO}UNASNone?é~£d»}?Ë«+õÆ1?ÊqŠm
?Ë«+õÆ1?âÓfÙA¿?Φ'¬Ñ•ð?ÚY2M|þ?Φ'¬Ñ•ð?éT·hrÁO?®'ç
÷¼?Ê­"^4úÅ?®'ç
÷¼?ã°Kóړñ?°êÙG…w?؟hJØ?°êÙG…w?é+ÚÏCõ?Ê
ˆºà?˓P"Âð*?Ê
ˆºà?Ák…#Ôæ?Æú(ûvÙP?륷?
Ç?Æú(ûvÙP?Øè?HY#÷?À6…i4z?ã‹à[Ón?À6…i4z?È/.²¬ k?³Œó5Ø¡?éô4ST÷å?³Œó5Ø¡MIXED4FGL J1848.2-0016?ã‹IJTj™?â™X {öÀ9@©-À:…! 8B@l¦Ð
ôà@Ó!_Ìr?ÉA¥Ãt?ÑâÊe€@XQeMa³?ñ´FÁZ}пïùÚí!+?ïðBRŠçO¿äg¿Sg†¿å`5•
Bß¿î/¢ŸÒ˜¿¿ïÿÍui8©UNASNone?ОëœN]?ÏÆk<l ?ç°òŠ1ØÑ?ÏÆk<l ?ºÍ®QÀ?»®}¹5¸–?ì¼J5Çý?»®}¹5¸–?ߛt?—ðw?¶v"›žG!?à2Eà4Ä?¶v"›žG!?ËLòô E?¬°©p|??é,ÜB÷ï?¬°©p|??³ëÊÚRs?·˜Ç¹|A?킆¤ì«\?·˜Ç¹|A?ƒÃ²Çeù:?"Øc9.?ï°ñ4¾¬+?"Øc9.?ÊäC‹ðå?³U•-B;5?é{†ïÇ?³U•-B;5?"AÿWM??x%šKIÅ;?ï¯Æ÷Ë©?x%šKIÅ;PSR4FGL J1848.7-6307?ìފíâÐÀ7³c€ßÀ;Ã2ú(OªÀ<ààðp@@!›?p-d'?ýÎÇä/¿á?ÐÖ€Ú?ªó/bN?מ§Šóäi?ùÅ¡²:$?ïÿùµc#¼¿ïÿùµc#¼?ïÿN>úg¿Ôú­ÛšðÝ¿æÏW´ü¿ÚTË^b¶ÙUNASNone?ïþÔ;«ýŸ?ˆ‹tiw…?"¼E;À$v?ˆ‹tiw…?ïퟻÐ-Þ?ld–¶oþ?b`D$Ób(?ld–¶oþ?ïë3g‹{?gÖ£§šÒ>?d̘qÀÕz?gÖ£§šÒ>?ïØÉíkË"?b%ýˉ_?s›	Y8·?b%ýˉ_?ïÿGUfS?/Øâ£v?w¶úVÏ?/Øâ£v?ïÌ£1¦t?kÉýQ?yñ.IÍô?kÉýQ?ïéQÅ£k?q¸Àba?f®ðÁlÞ?q¸Àba?Ûõ§?€ãåæÎԃ?‰ÚI2&Y?€ãåæÎԃAGN4FGL J1849.0-1826¿ìâÝK[YSÀ-s!_ÌÀ:hÒlHþwÀ;ä"îA'›@ÇZeý
@Ïw¡øì?Ïz!™­»?ÖÔx<ҙ@@¸â4=@In+ߤ?èÃêXÎÎ?ïû³4uR'¿à¶e)O…¿è@Åø50¿ê3^1
¿¿ïÿ¶>@£UNASNone?ïW Qñ1?"{ H$%?•õÓ!Ø?"{ H$%?í[¼mf¦?¶#—Œ'-?µ"–î×T?¶#—Œ'-?íþ Jsýº?œ)
£7¡.?°
ý­©ì¯?œ)
£7¡.?í¡:![fÐ?"RƒNŒR?²ö.õ'¼ü?"RƒNŒR?érè7êۉ?Àæ3N¼Ô?Ê4_ T'Û?Àæ3N¼Ô?äLtž?Ñc1ª¿S4?×ágÑÅ?Ñc1ª¿S4?æXIòR?¶Æã!ú†?ÓOËlÿ\?¶Æã!ú†?åI'–×-µ?º8ó¼zÅ?ÕlÚÒQ¤–?º8ó¼zÅAGN4FGL J1849.4-0117?﹗S¡ÆA¿Â¨†z'À8T‰.‹CÀ9ž¡´N`@¿Eß]H0@'–é»ñ?ä@¯¸k?·ùf³¾3?ùg£áñø@û÷­K'F?ì"\
G`¿ážä'åp2¿è°‡A}Mß¿æ†o»y¾2¿æċë[-M¿íëÏÇSHUNASNone3FGL J1849.5-0124c?يù¸æ?ÔÂÓ\¼w?ã:ƒ7ò#?ÔÂÓ\¼w?ë'jºR?ÃR¤<µ¾?ÁöUš·?ÃR¤<µ¾?áîh¡æ*}?¸0¦­Q¨?Ü#.¼3«?¸0¦­Q¨?íz	–·%?ž¥c¥æë?´/³LÎ-Ù?ž¥c¥æë?âDs¼)*`?Õ	ä;9£ ?Ûw‡­«A?Õ	ä;9£ ?Þú‹Fš™?әJ~(z?à'º\²³q?әJ~(z?âKÞ¦F®Ä?Áí9®bè?ÛhB³r¢y?Áí9®bè?Ûùuûbj?‰e¢yÆ?âENÊú?‰e¢yÆMIXED4FGL J1849.8-0952?×¾là†›™ÀŽÏÃøÀ:fc$'†€À;ʺà;>š@ƒ‹û¡K•@|{*BÊ?؇Ï!Éf?ï."²‡§@
†Ã%"?ùœbCÁö°?îxËrK!¿Ç<™"ü.d¿æэ'Mš¾¿ï?ërªAˆ?àc¯ga8)¿å­j0öBUNASNone?íÐ-‡w®?º:R ß²?±~"Ä°ƒ?º:R ß²?ÙÉ©*Êóž?ҏ̌ò'‹?ã+jš†1?ҏ̌ò'‹?ë-OÆmH?§­ôÂИ¶?ÃJÁÀæJÞ?§­ôÂИ¶?ë"/on?¶ØdIÝlù?ÃwçBCòH?¶ØdIÝlù?ç>Ó#lÛd?ξzAH9?тY¹&I7?ξzAH9? ÁyÝf¢÷?¶ÎD_ð?îóèb)•Ñ?¶ÎD_ð?á©þsý˜?¹8œ^`?Ü­ÜÑ?¹8œ^`?ʤu†¦#?ÊÞ"¯Ïç?éVâžV}÷?ÊÞ"¯ÏçMIXED4FGL J1850.2-0201?í@²3¿åg|`£®ÆÀ8ïcF÷5VÀ:#Mçê_…@ ´nÒñ	@ñhr° Å?ÆÎ8‡°ãã?‹«íë;³ñ?Ðô:$/³?þÈÍK¢Àµ?ÚºÔè$A(?ևÊ#ÐÔ¿éJÙ!ï¾ê¿éì°Ý­ð"¿ÝõÝ%O›¿áÛÇqC9;UNASNone?àfæ]±?Ք¤.jmÿ?ß2ä3Eҝ?Ք¤.jmÿ?îz¶(N0?±ävil>è?¨^¤š€þ?±ävil>è?ä?sJ¥j³?¸_g£æ@?ׁjµ*š?¸_g£æ@?îõ´Ìi¿P?ŠU!ÛÍÊ? ¤³:?ñü?ŠU!ÛÍÊ?×<9Â"?Ñ̈́âAB?ä|aãó¶?Ñ̈́âAB?çfáײK?Б­‹'ÄZ?Ñ2<P›×j?Б­‹'ÄZ?å#(üÁ?À2¢$é«?Õ¹®Ëâ}?À2¢$é«?çd÷NçªÛ?½;Þ+ޙî?Ñ6b0ªJ?½;Þ+ޙîMIXED4FGL J1850.7-3126¿ØÀ©ëmÄ À+@y€õ]æÀ:—žã…uöÀ<:g;x|@ùª&ڊP@ýã$ýæJ?Ò¡]•Ç?äÙ=ôWU@y…'Î?ú‹šZ‰¹R?ïêR^œ˜}¿·*1¬ËOŸ¿æˆ­'f¿çZ.I¿f³¿ïÿñ¢o+1?ê©}'QýUNASNone?Ý°hÿn­?ÏÓû{r"m?á'Ëø€Hª?ÏÓû{r"m?Õ»"pÿ‹?ÎY¤¹)Ï)?å"vµÇ€:?ÎY¤¹)Ï)?æ­@	QÚ¶?°$"@x»à?Ò¥í\J•?°$"@x»à?×4!1ueT?³:?¦eY?äeïgEMV?³:?¦eY?Óí «Ëd1?Î;택ü!?æ	/ªMè?Î;택ü!?ª¸ÎCÙi?½(¸'p©®?îTsdý¹?½(¸'p©®?Ó³Àºxiý?³_T5	º?æ&¢ÃË?³_T5	º?¶û:"œn?€Ø‹k´Q&?ï$íŽ?€Ø‹k´Q&MIXED4FGL J1850.8-1105¿áÜÝIwîÀ•?9ѲæÀ:yx˜˜ÚÀ<"u]@–ú©T@0#Á¦(?Ѹ:#gc<?éj܂Luú@þ"'Ùc´?üý"åø?ïüB"ßοéwKáâ8¿É*QwÁØ}¿èÑþåxÀ¿ì»4SÄ£3¿ïЋ¾dª$UNASNone?ÏrksQÂ|?ȪŸ·ç8?è#e#+a?ȪŸ·ç8?Áì8wëžõ?ÀµÅ$Èó`?ë"ñâC?ÀµÅ$Èó`?âps?4?Å?´Iiýrý'?ہ—€v?´Iiýrý'?̝LÆFÇ?©Öøð?èجÎn|N?©Öøð?±ó'¯*Ջ?¿M9wMœô?íÁÊ6"/?¿M9wMœô?"v¨E1w?¥·¬íóÞÁ?ï\J½­8ø?¥·¬íóÞÁ?Ê_µ@ØÒ?±Å/åù.?éh¯ÉË?±Å/åù.?"£éJ~?´*"És?ïgbàÓrŒ?´*"ÉsMIXED4FGL J1851.0-3003?é°ùærÀ*BÀð¸À:ö2÷¤À<;ê'Ù²@Ú<ü@:Ü$X¤Ý?ÁY«'zC=¿°<°	š?ò1r¹[@€
Y]¿?Ð=û"ˆý¿â#¸¿ëH¶‡D¿Õ][$éÄ¿ïÿü9¡â=?ïÿì»"UNASNone?îMhÐ0ô?Æs"X;ð?«)w¥º?Æs"X;ð?ïÃ2ê¸ðø?…ö=«Ô|?~fŠµe|?…ö=«Ô|?îݟÅÉg?–D칿8k?¢&Å[7‹?–D칿8k?ïá"b•Bê?YH^z?nli]=Õ?YH^z?í³qö?±™Uu?²dw_ô6'?±™Uu?íQCþÌ=?¼pæKgÌ1?µuàæI
?¼pæKgÌ1?î¤_ìàϟ?œS1üEn?¥º1ó?œS1üEn?î¤XÈK¼J?˜ýŒR÷-O?¥ºsx°†i?˜ýŒR÷-OAGN4FGL J1851.5+0718¿È‹)iZâ@
i‰¡ÑÀ9"5´í³À:ÆÃhŸý@°¯þ4ù²@ýˆ ËQ£?Àdlü'œþ?É":·¶æ@½[û©Y*?ùPx–Ó?íU]T™à¿âÄÜ=ƒN¿èº«'OP¿á`‰½®vË¿ïü¤ávR¿ïÿùµc#¼UNASNone?Þ*>À¸Ÿø?ÏÞ>†šÛ°?àêàŸ£°?ÏÞ>†šÛ°?Ä:íGÁ‹?ÀÀ¸!Df?êñ{®?ÀÀ¸!Df?ç'|êL?´;è‡'!
?ÑÐûü+h?´;è‡'!
?ÚÙÙXŸm?°ò­|½z?â"pÓ°I?°ò­|½z?º¿ÿð÷µ•?¼¸žÎÑy?ì¨á	M?¼¸žÎÑy?‹¾nüg8+?˜Å¶ÐX"ä?ï'D¤¯?˜Å¶ÐX"ä?Ö$"fvN?·Û."f?äíµÌÄØü?·Û."f?žƒâmàè"?‡hg â´?ïàìÇò{?‡hg â´MIXED4FGL J1851.9-1522?퟈—HmÀ6F(}‰À:zà,À;ä€Ø´5@Vœ.t\ž@ã7!Õ<Þ?Õ\ôb=ú?íþdŸfã@7Œ†‹ŸÜ?ýkûägs,?ïï˜p"¿Ñ7è‰ø<¿èj&Ìóc¿ërH½3«¿ïÿÚÁ,/´¿ä$ð_µUNASNone?âۂØÜX?ÐV'ZZ5ù?ÚHûÆNGP?ÐV'ZZ5ù?NJ¿ŽBDë?Åy‹ùGÄ?êPonÅ?Åy‹ùGÄ?è,ìˆ1šà?¯zã=U	Ã?ÏLMß9"?¯zã=U	Ã?Ȭ%B.Π?©lô>¤‰?éÔö¯tLX?©lô>¤‰?Ï7ÚNW"?ʙDcv
ã?è2	x,j?ʙDcv
ã?›êœU?ª
æ™7Û?ï ¯×^è?ª
æ™7Û?Ô²ˆuQ]7?·%o@?妻ÅWQd?·%o@?'e´2IÅÆ?pŒ]#M3N?ï¶i/]T‰?pŒ]#M3NMIXED4FGL J1852.6+0203¿îʽLŸ?åcl2š‡À8
 yóÀ9îäùê<I@^ô­™Ö@¬À½ÊÑ?Àâ3{ØhŒ?ÃK¤n3å@o‹XŽ6?ó,c8¯ý?ã¥üH»Zµ?Ír!²lN¿æv÷"‹Æ¿è¸€å¿ê–ß~*R¿äîDنUNASNone3FGL J1852.8+0158?ÝVG´8p#?Õ¥Kùþ‰2?áTÜ%ãÇï?Õ¥Kùþ‰2?pn]?Âd©|)‹?ë`ãؤi?Âd©|)‹?Ù@	8?¹[E%B?ãpýßûcõ?¹[E%B?È´>¥?¬[ì›ã?éÒùà0W?¬[ì›ã?³W(…Û Í?È÷aJó™?í•ïD›æ?È÷aJó™?‹%ʌM?ž›;¸\
?ï"ëÏhÕÏ?ž›;¸\
?ÎÈ"4œ•?½‰Lߊ?èM÷rùØÛ?½‰Lߊ?'ZxÂ?R?rœé˜%t?ﶖÀË?rœé˜%tPSR4FGL J1852.6-1159¿íÇÄQþûHÀ΢(´TÀ9çrüvބÀ;p££×e@h¿:­@Zñ£EêÆ?ÉSme^(ª?Åö/‡,.²?ý[ö Û­?øäC%ï}Ò?ïÜ5?ÒÓÍ¿´¨JŒk2Ô¿èûù`(´ª¿âwÆ´{G¿é¬lÚô­¼¿ïÿ¦<ådUNASNone?ïSF€W¡?¢wÐÍ®u?•—=µuå?¢wÐÍ®u?栔ÁSÙ?ÇëQ[oñ?Ò¾Ö}XMý?ÇëQ[oñ?îY£r¾ìî?šTö_>ë?ªeÈÕÈÿ ?šTö_>ë?ê¼L:Úá&?¡±!t¿¦'?ÅÏ"{f?¡±!t¿¦'?æÈ·±TÒ?ÅÑ´n˜JJ?ÒnWÐ]?ÅÑ´n˜JJ?ÈõÄìóL­?ÉLf©
–?éŽÄÃ,Õ?ÉLf©
–?å$Zéõ–?»}ëWT?Õ·KÎ,Ó?»}ëWT?Ó$Ù³åö?³C-ºì?æm"&
ö?³C-ºìMIXED4FGL J1853.2-0922c?íó³&;0¶À¬¦¡¿ØÉÀ9ËÇ;"TÀ;MC0×8a@nLÂ{e&@®qÛ®ï?Ò3Ȅh¯í?Óø[{¦¿r@j ÒH7?ú¥mL¿ïÿÈ‹ñ:?ïÿY¢Ò1¿î2ái<¼¿ÁÀÒº[Ü¿éâÅA¾q¿ïüí'hr°UNASNone?ëßîSÉðh?Ã"!["6?À€F°Ø>_?Ã"!["6?ÞMoOd?дZ¶Áû?àÙ9H1XN?дZ¶Áû?ëS8êÐ?¨yì!ž,É?γÏTÂ?¨yì!ž,É?ç	¾DÉ´?±•TçWê?Ðåìƒvl™?±•TçWê?Ù\…"U!?ϐHd?<"?ãQ½=ýUp?ϐHd?<"?¿%;p:ó?ǘþöâíB?ìÛX'ø¢?ǘþöâíB?à¼ÊbS '?··_ÎjÞP?ކk;Y¿±?··_ÎjÞP?»$›_c?°ºxŽŒ[?ì›l"T?°ºxŽŒ[!MIXED4FGL J1853.3-2447¿ÌyBƒž=À&Û¦&oÖRÀ9ýìgpRÀ;µt1*Dw@ÜÓò0±@Ôa0œþ?Æ\ÜdokH?ÅҁGRÐ?ø8¸®1×@Ÿä6v?íê­ÞJ"¹?çßùÀë-¿éN¯{㦿ç–j€˜A¿ãi!—)|ѿ䍍â?UNASNone?ïÆC;œ–Ø?{üiŒOs?|ÞbX|]?{üiŒOs?ï5ú–g=¯?¢Zƒª"÷?™@­;¯P?¢Zƒª"÷?ïÒd2ÑÜ?'àÌc9n?E³€"ü}?'àÌc9n?ïê&œC?áµÃ@?ÿ»,w"?áµÃ@?êa—ÝàN?ÅÌF•Ç?Æy ˆ~Ǻ?ÅÌF•Ç?éW'îuWà?Ê*Jª%áo?Ê£`F* ?Ê*Jª%áo?é¤J!·?¸÷Ÿ‰G¼Ø?Ë»õn×y#?¸÷Ÿ‰G¼Ø?é¢+Ð=p?±n柳n?Éw—P¿
A?±n柳nAGN4FGL J1853.6-0620¿ç Gñä¼áÀ*èáÖIÀ9ÞŸ]'ùÀ;6â¿}Xñ@Ô¹¤{õÅ@ÁŒý©äj?Äá…@œ'h?Àí·(Ùº?øLZ·»+@ÿµ$¿ïþ;?ïÄÒݲù¿è‰áØT¿ß¥ý THØ¿ïýÈ[fX?ïB€®IUNASNone?ïé=¯Ÿ%±?vnùX+{?fÂPy—?vnùX+{?ï!>=O¼?¥ É‡Ê™?›Ø8]6r?¥ É‡Ê™?îs'™:èÎ?šÝ1ùì"?¨Í†i½¾$?šÝ1ùì"?;§\?xUr«¾?;š{düä?xUr«¾?î'(2	x¶?¬ßo<¨ñ´?¦í|àD[¡?¬ßo<¨ñ´?é>Åñnö6?Ì×5ÓÃÙV?Ëè:D'*?Ì×5ÓÃÙV?é¦V³bdñ?¶'±6í?Éf¥2vl:?¶'±6í?ë"ҍ߅?´¾Üí‰ä?ÃÍ°µÈí?´¾Üí‰äAGN4FGL J1853.8-1107¿Ò
Z
´ëÒÀT#;z*À:TóRr"›À;‰¼9Ҏ@méLµ:_@¼7£~ö@æ|­_I?ç!J}|­{@'«¹VÎC@%ÎÚÄU?Ñ@|g¯'?ï{ÝáÈ"¿çÛ'£²ø¿ïà.ʖ<?í®ñðs¿Þ!§ÚúâàUNASNone?î'8µ.?À~FéËM?®gÜ|%?À~FéËM?æÀû²µÁ»?Õ1à†×¹Õ?Ò~š"|Š?Õ1à†×¹Õ?êäÐK~Ðã?«Þo}	—¹?Äl¾Ò¼u?«Þo}	—¹?ï#Oíu†?§†ýRÚ %?›ŸV	0‡0?§†ýRÚ %?ëþ
0UÖ?Ç#¥vœ"?À˳>¨ª?Ç#¥vœ"?×'ß(UE?×¢N‡U'?äplkÕ^?×¢N‡U'?èh«=íº?²U1ÐP¤?Î]SKå?²U1ÐP¤?Ý#tB‹Û?ØL±$‹á±?án~EÞº?ØL±$‹á±MIXED4FGL J1854.3-3640?¶{¼šÇ×À0ZÅ;ËÀ:ÈPÓW*‰À<SAÞËÓ@$cb@.ø; ‡?Ó"ë|æ/Ÿ?ÔKÖãQª@yÀÌäJ@WIí	?Ðe0pá¬?ïîh(†¿á…ô¡'-¿Í']êâ¿îuLþ`m©¿ïüþy×ÝUNASNone?ïÎÁ,–È?z±ú¡	è?xŸiθý½?z±ú¡	è?ïüå曢?¡rPð×p?œÀcJì?¡rPð×p?ÄÚ²?""j͘Ã?§·>¥j"Ø?""j͘Ã?îËö+Ñü?…¾zî>?£@D˜0?…¾zî>?ïʈ}:œ?óÑÝN˜s?z»Á¿i¥?óÑÝN˜s?í¶Wщ[?¾sFQP³)?·M?Mó©?¾sFQP³)?ìÇ&TÓkø?¦ü%Ôöô?¹ÆÍYd >?¦ü%Ôöô?éfiRBܸ?±ä¨ek=?ÊfZ¶ô?±ä¨ek=AGN4FGL J1854.7+0153¿ìñԜW—Ÿ?¾·¨£L˶À7ù$(Ô4 À9ßc¨F@ÙqóbbÌ@3‹Ë{?À^®÷yɛ?Íà*w¢Ï@\E˼+•?áh­éæ@Å?æØq
"=¿ç'ö?p¿å/< B¿å»bó_¿ê†È½¯#¿ðUNASNone?ÀÌ(7+»E?ÏfH€Ä­ç?ëÌõò5/?ÏfH€Ä­ç?£Å"k®Ú?§$}މ*?îæÉ`@?§$}މ*?Ò¶L˜u?³r.íbË?æ¤ýÙñ3Æ?³r.íbË?…´x‰´?unÿ9R?ï©/îI
)?unÿ9R?ÃAXš Õ£?ÔWÔ²õ5L?ë/©ÙWʗ?ÔWÔ²õ5L?u4ñ¯Ô>?ƒïFÞÜ{?ïՖýÛ§?ƒïFÞÜ{?À™uØ_?«¢¸Fý·?ëÙ¹âºIè?«¢¸Fý·?šÎ{? ?'ÅΙm|?ïÿ;)KÓ¾?'ÅΙm|PSR4FGL J1854.9+4054¿ÀÌ&Vçÿ@0Â!x÷À;>D¬Ø:¿À<jV´A»Œ@þD<ÅÙ@Ñ¢£Y?É[~€äl¿šGÚ<Õ|?ÓO*_¥,?úZu—[Ѹ?±¹YÓ[a¿î³
=Ö$d¿æ@sÝGn?Ϲ¢x`¿é\n•à¿ïÿÿ²}@UNASNone?ïòþ[©ã­?SµChgv÷?ZI,$l?SµChgv÷?ïÜÁufð‹?|C³ã	¸°?qŸE;Y®ƒ?|C³ã	¸°?ïÊP–Îì•?xµ¹Sµ=?z×´}¼Á?xµ¹Sµ=?ïÛ.,
O?\ePýdÐ?rhéòy9?\ePýdÐ?ïÓsÿùl_?rd‰Ú"n?vFçx+?rd‰Ú"n?ïczrÚ4Œ? QÐ4£Z?"±Ÿ'Ž? QÐ4£Z?ÎÎÉk?ˆKýœ‡çi?‰TLS,Ý5?ˆKýœ‡çi?î×ÊPèó?•=Wø…$|?¢ƒZòLµ§?•=Wø…$|AGN4FGL J1855.2+0756¿íQ<ï°¹@/«NiÀ9µÕ×7‰ÚÀ:Ž~ŸBP@!ÑÞÚkq@íê‰v5ç?Æ£Þ×fXÏ¿¥Nƒ_ŠBþ?ç§Làƒbö@±ؚ‹\¿ïчF°¾y?ïÿl'ù'(¿è‰î@dô÷¿ëž¾°nÈ¿ãëæŸ‡?Ч÷à÷§UNASNone3FGL J1855.6+0753?ïnWÕ¶?±Á xôÈ?ŸÒ5ÎÅE?±Á xôÈ?ïqµt¢Ù? j	åÛ1W?'É_JŒlë? j	åÛ1W?ê\°a²"?²ée'è]?ƍÁ>y7y?²ée'è]?ïÜcýš8ë?c=þ{Ê?qΆ2Ò?c=þ{Ê?îÃýÜAè`?¨ž"B¢ð?£À"9MÄþ?¨ž"B¢ð?ë\ÑÔÀÙq?ÆP};?I?Œ¸¬üš<?ÆP};?I?ë>Ÿ€–ò?²ƒt!y1?Á¿ý¤9?²ƒt!y1?î>Îÿ?Þ?¥´s€#~?¬£{ž?¥´s€#~AGN4FGL J1855.2+0456?ïí5š°_?ösC>C1®À8(ܛvékÀ:ð)É'&@\àb€Ô@¦»Ò©†?¿õW°kP?ÉPx‹H@Šu¿Ÿ½ @Ê(K£—t?êœËbi¤¿Ù߀®'¿èº°ÕöA:¿ê¹ËhH¿¿í2Û>Õ}Ë¿ïÿ8$3»ïUNASNone3FGL J1855.4+0454?Òb¿)~˜?ÒÔsʨk?æΠ|ë@´?ÒÔsʨk?Á®ãmM5h?Á:%yk.?ë"G$¬²¦?Á:%yk.?Ú{ŠSÅ=Ñ?µç2Oܬ×?âÂ:Öa?µç2Oܬ×?Ò²IÄIþ?­¾ïw.c?æ¦Ûó[?­¾ïw.c?šÎ…Z*@?´÷äÛ9áž?ï)óþiþ?´÷äÛ9áž?‡I…¿xúˆ?šá"¦F˜?ï¢ÙèØàÆ?šá"¦F˜?Äq&•¸Zò?¯sÿõ Üw?êã¶Z'éC?¯sÿõ Üw?‡\üUÇ?tl"|O†?Çåm"?tl"|O†PSR4FGL J1855.3-0740?Ƅq¥<nÀgϽBNÀ:$ÀwSôtÀ<…
š¶@#²…£Ã@2ƒZ'ó?Ò͖‹È¿?ﻜÞÈwÓ@5ÿñ?ü€…S'wŒ¿Ó:9LQè*¿ÂùCbÖ9¿ãle¹˜<¢¿îUĝ~U›¿ïùzu$?鉸 šê§UNASNone?äW–O•È?Îñ;äT^?×PÓ`Ôoó?Îñ;äT^?¾Îò8c–?Ày±qҀ?ì&!¸ó<?Ày±qҀ?â™7·¯âº?²âËùê?Ú͐ :Œ?²âËùê?ÉþýŒŠ?®ºyˆ ?é€O?МÝ?®ºyˆ ?Â?åÜpâI?ÇUïýÅ&?ëpˆãÇn?ÇUïýÅ&?Š"9á"1+?š瘆óD?ï—wBõ|?š瘆óD?Ã67ñC"?¯|°ºv?ë2r¹¯?¯|°ºv?€sÉbùa8?q'Ácçï?ï¾0Ú4á«?q'ÁcçïMIXED4FGL J1855.6-3603?î[kǵqøÀ0\'IðåÀ:ý6¤û©À<©"¾péw@ð$ÃXÚ¸@	üD~?Ò2µ^ñýß?êb–P@žӕ=ê@-}C¢—?ïÈb¥Æ!?ä̤S0ÿ|¿ØPêh¿;¿éÛÑý¹(Ö¿ïÿi'_Ž¿ïùõ÷h'UNASNone?Ü"qy¿ß?ÑY=íæÚ?áîÇC A?ÑY=íæÚ?҄p_Æ©?Ξ«v'?æ½ÇòP¬?Ξ«v'?Þ?Nr\qy?³ìazŠ
?ààXÆÑÇD?³ìazŠ
?ÄL¢±¬q?¦G®D•i?êìýS"ä?¦G®D•i?ÏJʜ¤n'?Ð_D¾tx?è-MXÖä[?Ð_D¾tx?«É °vP?¼¿õxèt?îCe÷;ò[?¼¿õxèt?˜g­ÒÅ?«"Fß½‰F?ëYæ¾ËO?«"Fß½‰F?‹ž›d‰'G?}
Y±]kÒ?'6ß÷?}
Y±]kÒPSR4FGL J1855.8+0150¿ë×Fà¡¿ÁvN{c"ºÀ8¢ _ñØÀ9º`Ðû/·@ `7ûÄÜé@ܙ®'O"?Èajh©Œ¬?ÐZãü>T@phÌ›?ýq¤Ýð`¦¿å‡´Nß¿ê#| âΗ¿ÓË ¥<%¿å^ÂÞatº¿äè,ÿèX¿ðUNASNone?ÕÓò¹y–?ÓÊ?óÏ´Í?å£Cwµ?ÓÊ?óÏ´Í?Ê'!Í/HB?È^ÖšÚ?év7Œ´-ï?È^ÖšÚ?Úâ]Rk‡¸?¶ÊOÉ?âŽÑVÊ<$?¶ÊOÉ?á°Õ×ÄÈ?½Zÿ勤?ܞTQÄvp?½Zÿ勤?×Ùµ%ï±\?ÔSZ<?ä%m'R?ÔSZ<?ŽUÿEX?ùXXøî?ï‡ÓªÑ>:?ùXXøî?Ünlä?¸åúÂQ¿R?áÈöw|IŽ?¸åúÂQ¿R?¡èÖó¶(m? 8Ç|?îár£¹? 8Ç|MIXED4FGL J1856.1-1222¿íg/!´8À‰"š|À9Èé<oÀ;¬‰RúxØ@nýúÂ("@ƒæœ«f?À±ÿ¦™?²Q_>e?ô'|æÛkÌ@5ՏºÉ?é2^ASÝM?ï´6Óѣ̿épÔH±¿Ó'C>™ê¿åÔcšL¿éºžÌßADUNASNone3FGL J1856.1-1217?ïðèßõ?"J‰Â>Z?_ÕúŹ?"J‰Â>Z?ïZ
›mû? VÒ
?"¾¬¦²°? VÒ
?4݇{
?gM(i6?€ÚÙ˜›?gM(i6?ï^ÖºŒXh?zERáI"?"%(®tòñ?zERáI"?ïr¾®"?"O"3xJ?'¨*C/¥?"O"3xJ?ì›
ç~m³?Á²‰ïFc?»'¨Ä'h?Á²‰ïFc?9i¥'? º=pQ`k?¦f|eöÝ? º=pQ`k?íRÔۆp?¦áÏDI¦ª?·MiYÿ³|?¦áÏDI¦ªAGN4FGL J1856.5+1735?à˜k׏É@R§¢pØ°À9¯0YddÀ;šätªÍ@žç'–òË@ù?ò^VÍ?ËéÖš9?Ïèw"KYp@Åã|;ºÁ?úqòxØÙË¿áZ΂¯rI¿æ¿‹€Ò"w¿åj¤ï81 ¿äªÅ 0!0¿ð?ïýk›Y:UNASNone?îÈÓ]ùA?¢p®œh´?£rϖ°Ïú?¢p®œh´?ë<ºèÁ?Æ/¾¥}ä™?÷
\û¦?Æ/¾¥}ä™?íĹïê"?Çð-Êʆ?±Ú0øÊ?Çð-Êʆ?í²?³Ê?™ýy'èûW?²oŽ}?™ýy'èûW?éMò¢¹?Âv§íþÔ?ÊÉø5u¥?Âv§íþÔ?ÍÃx£ˆco?ϦFÛ܊/?è!×ç$?ϦFÛ܊/?â	9Ò+'î?¹C§˜Iˆ@?ÛíŒ[©°#?¹C§˜Iˆ@?Ü þÇ_"T?ÀDïWUJ?áP5Ö?ÀDïWUJMIXED4FGL J1856.7+0125c¿ï	i‰—ª¿à³PßìdBÀ7–|ÿ/¨À8Ö5¹ö0s@ÀÈGW@u üÏÊ?Ï(ퟀ8u?Ù&݄ªõ@MI€|'"?úCˆ¸Ë¸ü¿åە"d~?ïÈpçɨU¿Ú¬)žßԑ¿çÝÊD\P¿ïãÈ&tÞÏ?èëï<c]UNASNone?ÏâãÖ¿?Ñà7¬ÙV7?èzG;JP?Ñà7¬ÙV7?­'¶™¨´Ê?®æ<?BØ?î'Ԗ€ñ"?®æ<?BØ?ÕYÍ/Œú>?¶¤½qâ†Î?åSh9'á?¶¤½qâ†Î?²—sΩ§Ì? vÁ!y˔?í­†N'? vÁ!y˔?Ðó¦e"ê
?Öå»ýœ£?ç†,Í=Šû?Öå»ýœ£?yjiw]E?†±B¾ÒŸ[?ïÍÃ+R-
?†±B¾ÒŸ[?°Låå¤>v?©k?íöcC=¹Á?©k?Kqؖdz?DóÔ¨2_?ïù#¼êùÖ?DóÔ¨2_4PSR4FGL J1857.1+0056¿ï½¾¨'ü°¿ë-4¶ÀñÍÀ8…äÅøÀ:c®ƒ5ª@ ±—è¥@[ àJX?ÁºuÝ&â?Úg§cܞQ@9Úak@Ò¸¯3‰Å¿ïý*,ú4?ﯴޙ}ë?¦tûTŸ"…¿ã«ón!EË¿é-¯›cž5¿ïô‡'YY8UNASNone3FGL J1857.2+0059?¬[h€Vƒ?º"þ×®J?î:G	\}¸?º"þ×®J?²Õ	´ÄQ?´w®7-?í¥^É0'v?´w®7-?Ë	å‰(ª'?¯ÜÌüµ'?é=†µÕ\?¯ÜÌüµ'?Áºaî»Â?¤dȪÉÛ?ë'g"Q;?¤dȪÉÛ?|ڔ8Ìk?¬ m¾{é?ïÆJ×ê'?¬ m¾{é?~p~/?Š‰ÉÞT
y?ïÃÏó¢?Š‰ÉÞT
y?²ôEyÁ=÷?«Är¡?í¡wPÞ?«Är¡?{*èÏ [?o}C¤ë•?ïÉÓ©ñç ?o}C¤ë•PSR4FGL J1857.4+0106¿ïöq+;m¿êmjf¦'GÀ9¶)XüÀ;%ðÁž›a@ ¯®ôŸ¥@—á¸íø?Јñz+??ïÜ`w	L@h½=ã^?ó"ˆñ*Ð
?à'5Œ©Ç¿ìؑ[Ývh¿ÔbI€ýk{¿ÒtDöT0¿ì³L=pMñ¿äëIº^UNASNone?¾îI"¢†?ÆÔï+؇&?ì"6Û«¯=?ÆÔï+؇&?«ò{ža?®ò!Ý)Ï"?îN0Ø .?®ò!Ý)Ï"?Ù¸íiFâà?³^ê…À*?ã#‰K\Ž?³^ê…À*?‰ÛQc¹§›?x}Ó#UÖ?ºqb?x}Ó#UÖ?Á‡šþôgF?Òðä"#'?ëž@Bæ/?Òðä"#'?zY ó¦•?‡(}6\i€?ïËM¾P‹?‡(}6\i€?ÏàoKx‹?µ´ÐÌᚏ?èýä-!Ý?µ´ÐÌᚏ?<½J™é…?3ü(߅J?ïü|ˆšKy?3ü(߅JPSR4FGL J1857.8-3220¿ã%y™ž÷ýÀ.¹<FØ+¦À:#õ|ï>èÀ<ëD‡Ž@Œé‡îv@†ó{??ÄoÒ Ì=Ü?Î0/ȚŽ@¢"›R×=@¥¦Z?ï'ãt®þ†¿â†?ʛD¿ãø]߯' ¿åóÂ[.пéâ6'¿ðUNASNone?í¼Ü­¡?»M͆cºm?²¡ߌý?»M͆cºm?î¤Ð.?±Âô%Q)[?®Ŷl³é?±Âô%Q)[?îe½oÈËò?›o…áæ@e?©¤)¾ÃÓ?›o…áæ@e?íÇgÞ
·¿?ŽWv¹Žº??±ÄÁ<N‰?ŽWv¹Žº??æ5b*©æ?ƽÌIN†?ӕ;«Ò¬5?ƽÌIN†?á·¤±¿?ѶæŒø‡¢?ܑ·úœƒ?ѶæŒø‡¢?å}SIËr|?¶O­¦ç–ð?ÕYli?¶O­¦ç–ð?ãu(?²"Æô|±Z?Ù÷áÖý±?²"Æô|±ZAGN4FGL J1858.0+0354?ë Èxp·?Óу€R ·À7òŸûÆÀ9ß:Q4¥ú@*ÜGéùƒ@@öÍ0 ?º¾Ä÷@hÑ?܆—^Uö­@!
hn~bÜ@dªõ°7¿ç¿sFS¡¿¥ÁÍBC‹¿à'" ÔÇ¿ê_@z¿îJ}ғ¶¿ïðÌö%ŒUNASNone3FGL J1857.9+0355?²ô\_†¶?Á3©©öÍÁ?í½!t«é?Á3©©öÍÁ? T¥!KÏî?¢kTMA?îúµ®"<Á?¢kTMA?´›–FÜeû?¥t1ïÖ?íl7i+p?¥t1ïÖ?£Äý
²U?'ÌÁm'z?îÿø[?'ÌÁm'z?qÍàGÑÄd?§ª<NñÇÜ?ïÜd?£6¯?§ª<NñÇÜ?qª	q¢hx?€/Ë{:GG?ïÜ«íY4O?€/Ë{:GG?ˆ«·³í4?zpfý]‹é?ïQ!ZÛ?zpfý]‹é?8êd¥Š]*?0ð6‹Ÿ­?ïüâ³Wʆ?0ð6‹Ÿ­PSR4FGL J1858.0-1052?ÙD¦HÍÀÙý6÷äÀ9ØB/OxäÀ;U/‰Z‡5@ý¸G"¤@dÐd1@	zg9Êüé?à7½½eQ@Y" ä¶?ôfxÚÝ1?èc]c2¿Øì#"¿ç_¿ž ß¿èÄ® 'Û_¿ê"•%–'~¿ä¤²Çë¼UNASNone?ät¤Ýo‡L?ғæõ ‰+?׶E ñg?ғæõ ‰+?ϔò=Ó'ã?ÏfýŸ¹ª?èÃp‹6?ÏfýŸ¹ª?èš6´¿\C?®,ýT©à?͗%-Žó?®,ýT©à?ÒĚCžd?Ê/ÿՖR›?杲Þ90Î?Ê/ÿՖR›?×Ñù:¸K?ÒKÛÃ>?äbò#Û?ÒKÛÃ>?¡µ{* n?²KÅ<Ÿ?îæ$¨¥Ê?²KÅ<Ÿ?Ù6F³~Ù?¶m'c¹9§?ãd±\¦@"?¶m'c¹9§?‰6xæZb?ž5Ž®Ð\?ï›ÿ&*%?ž5Ž®Ð\MIXED4FGL J1858.3-5424¿ín\´sÀ6¹øã¬cÀ:*z¡†ÍåÀ<jñé¼Çœ@µ[ d¹é?ÿyfâ?¾ét£@‰?ڛaðµà!@?ŠÒVy‰@öýÝ;?z!.N¿ŸOZ±&~¿Û9NÀ­YÀ¿çㆢ›öÁ¿éA6ÌD瑿ïó³KUNASNone3FGL J1858.0-5423?ßh!Q‰`?Ñy\ÉjÔ?àtËïW;P?Ñy\ÉjÔ?æ&*Ô|Ø?Èô	e&Ý?Ó³ªWéP?Èô	e&Ý?à_œE¤°?²øPb‡ÎZ?ß@Çt·ü ?²øPb‡ÎZ?êçê=(³?¦¥ß·°çÜ?Ǹ`W]4?¦¥ß·°çÜ?§•x͜*™?»‹É&É?s&=V?»‹É&É?ÉWCécÜH?È­Œbôš?éª/§î?È­Œbôš?Ä)!•»T?´Óԕ̎?êõ·š¿+?´Óԕ̎?Òa…W(—	?³7÷ñœBŸ?æÏ=Tk´{?³7÷ñœBŸMIXED4FGL J1858.3-1318¿ïUw©ïÏÀŸU›=À:`þԆÕrÀ;÷ˆy¶¥C@Ä2¸V@ˆÏa҂ï?Îà'&ˆªß?àFƒÂ—¿¥@¯-šlþ0?ó	ú…Õ¯?ïöëN˜ˆ¿Ñ‰¦ÝNû¿äŠ&_Z¿æ,zFíû¿ïÿ®k¸µ¿¿à¿Z=¹UNASNone?Ú'Ø<¨¹?Íì¸`ÀEf?âìá«£?Íì¸`ÀEf?ÂdsgUϕ?Â*c‡Jë?ëfã&*Œ?Â*c‡Jë?ækrÞތ?±u;ö?Ó)BBçþ?±u;ö?È»ïod÷?¥6QžùÃ?éÑ$&ûÂ?¥6QžùÃ?ÁÔÝiŸxM?¾ˆ†ÛI	?ëŠÈ¥˜!í?¾ˆ†ÛI	?™ªÐs©?¨ghÑÈ­?ï7ʯf4'?¨ghÑÈ­?Æ=c~»­ý?±Ūˆn?êp§ Q?±Ūˆn?âCzªËX?kö]ñID?ï¸vñù×ó?kö]ñIDMIXED4FGL J1858.5-4446?ïç–ØM<À3ì«Oœ À:vW&WƒÀ<X£Ò¿ô@²çÑ`x@ó8ÜÀ_×?Ç«µ¥é´?ÐLI'@ÃÏ,ù]O@ˆñ«©g?ïþaßîé¿àv'=\á¿âÑD£ÿ¿çg)ÚÄÝ¿ïüÍ{Hu»¿ïÿÚ@RÖgUNASNone?ï£Jß(¼?ˆ—_Ã$?‡-|ýæüø?ˆ—_Ã$?ï™üæù|a?'Ðßä©"Ô?‰€Æ3âwÝ?'Ðßä©"Ô?îºV•/t?•ÜUb?¤Z–­¿Ë?•ÜUb?ï=;iš?zœ¿Ù"Dg?˜Xº‹b¼?zœ¿Ù"Dg?î"\ãÓ?±\¨ëy¾»?­Ú1ê5ß?±\¨ëy¾»?î€7Î"I?´
UQ<Ê?§üƒ×+u?´
UQ<Ê?ê:×Jè?°1Ãkîô<?Ǔ¢×äa?°1Ãkîô<?됤û]À?¤D"P%óŠ?Á¿Ýl‰?¤D"P%óŠAGN4FGL J1858.9+3636¿à4ÃJåMï@,Êl¬Ñ…À;l–+PÀ<¡gSÌ/ï@¦å‡ƒÂ@ÀµgU?Ñp˜ïO®"?äý t-Þ@?ý¾Ý ?ü>t.ûì?ìÿ¢AÞÇ¡¿ÍÛF7Fé¿áò?£%¿èñ¡Þ6¬¿ïþ' ¦Ô¿ïÿþˆ0»ŠUNASNone?â¤9kí ?Ê¡qGs¢?Û淍($À?Ê¡qGs¢?ÓÆYî*aö?ÈY¬ê¢~?æÓêÏ?ÈY¬ê¢~?妑T¯7n?²Êp°æ?Ô²ÝV¡'$?²Êp°æ?ØW	&Db?¯+Žc°~?ãòÔ{lÝÏ?¯+Žc°~?ËF€š¯G?ÂæÂ:?é._Ù{Ô.?ÂæÂ:?©Õ+\xq™?°x´UK{?îb­Ja´6?°x´UK{?Ê¡Øø-2?°Î†"ر ?éW‰Áà4´?°Î†"ر ?¥ÊI?˜ÆùôÚ?î¯#vì_?˜ÆùôÚMIXED4FGL J1859.2-0706¿æن]k…ÀÒiߗª¬À:M5fêåÀ;º©¢%YV@yc%¿,P@c8´|sï?ÓÝÂ=|¸?Ø\ø¾îì@	¦~â^.Š?ýrö6þnÛ¿ãÌÆ폻¿pjwÜÊ4±¿äÙÝ¡‰¿å•;ÁL;¿ä'̘ÊfÁ¿ïÿOÖ×èŠUNASNone?îo
/y¦p?¦Y%¼ Xð?©-õý?¦Y%¼ Xð?Üó·>'"?Î&dߎׅ?á†u¤`¶¾?Î&dߎׅ?í¢¹d?¡½ü‡Fþ?·/ïÆÞ?¡½ü‡Fþ?éM±‹u6?©öã©` ¥?ÊÉ9Ò+'î?©öã©` ¥?é𷜨±~?Áw(VéÏ?È=!]:?Áw(VéÏ?°ìSg–'?¼TÉy
æ{?íâu"Uî?¼TÉy
æ{?åKw2øŒ?µ<s׳ȩ?Õñišè?µ<s׳ȩ?ÁÙÆI>Ò?­"	ÝQê?ë»ÉŽm°K?­"	ÝQêMIXED4FGL J1859.3+0058¿ï§é_niY¿ôðT@Éô«À8ƒÅL¥ËÀ:7m´Zæ@ ,½¡W(@N&&v‡?Ć<¶µ^?ÈÍî_ï~Ó@•;Ãûló?ý®àË¿ïÿï~Óo©?ïÿûB«÷¿ásœ¯ÎE¿åm_[°¿ç'sýþž¿ì>†ƒ<`UNASNone3FGL J1859.6+0102?Ø´sÀb?Ó:ÃZ™e?ã÷¥ÆxŸÏ?Ó:ÃZ™e?àß²¤úÃ?ÏÝ%\8™?ßÔ@š¶
z?ÏÝ%\8™?ÚÄ"®4?»âaK?âþ¶(ñf?»âaK?ä†×"nÈh?µÒ:Vqé?ÖòQ»"o/?µÒ:Vqé?ÇN'YŒ
j?Ǥ¯é"?ê,_iœü¦?Ǥ¯é"?ŝgt?ËIîöî3z?ê¾Ø¹¦:£?ËIîöî3z?ؽ8çõi›?À¶Ìÿ¼R?ã¡cŒK2?À¶Ìÿ¼R?½=—æ?¾?°îc‰Ÿøð?ìXM=ø?°îc‰ŸøðMIXED4FGL J1859.8+1545¿å±ŠÙ"¸ƒ@-ÙÝV‡ÌÀ:²€Þ·°ÜÀ;"''Û\@ •ù&rª@Î!¾–©$?Äk6D_«a¿´à!tK×?ó߄•%–'?ÿ«›úœê¿ï@†}ˆ?ï1KgŸV¿îû"‰µ ?¯•pkwó¿ÓûpcÀCÒ¿ÎÐE藃•UNASNone?ïíÁÞv[?¶ù"ÆbÍ?b>!³4ôt?¶ù"ÆbÍ?ï0
îµC³?ª»Xˆ¼®p?™þ¢)W‰¡?ª»Xˆ¼®p?ï'=~Ýøæ?‹¬Œ3¬49?p :ÃVt?‹¬Œ3¬49?ïEó]?VÄÎZOY•?a{\ìæÚ×?VÄÎZOY•?îÆP€îIl?¤õݗiKp?£š÷òÓ7C?¤õݗiKp?ꃁ¡¢Ÿ?ʮ̄†µ?Ç¥ñùyu"?ʮ̄†µ?î2PExì6?£36¤†ül?¬Úû§•Už?£36¤†ül?îá?ä­¥P?ž}Q/4°h?¡ì¸•Fô?ž}Q/4°hAGN4FGL J1900.4-4941?»Û 2áäÀ5½Å?9ѳÀ:öwZªpÀ<‰Ü°ožô@ëzPÔ@üÁr&?Ï8D,ï?×øúRAt@	ޏh"@p¾®üØ-?ïû¼¤`œù¿á§±ŸÊ¶¿ß[Á•â¿âg)¿ìêz¿ïþÕÞn_Ú¿åSu}°"îUNASNone?wEÜ®?Œï®§‡hÌ?‡âZȒ?Œï®§‡hÌ?ÁÞ¡?"_++^1?àÅ9ƒÐ?"_++^1?îš>Üò?"Ïz0…Ÿ`?¦\@žâ?"Ïz0…Ÿ`?ïZÄUɤé?sÛ¿ÅÜz`?"§uJ:þÝ?sÛ¿ÅÜz`?ïD;âÀeG?›šŸ¶»©¿?—xƒ®Ò$?›šŸ¶»©¿?íª/©eêk?ºx-ÆQf?²®'¶ˆz©?ºx-ÆQf?èÃu"®š?¶EddÛN?Ìò+ûuE–?¶EddÛN?뵖ßCá›?¢«ÐýÙÁ?Á)¤'ðy"?¢«ÐýÙÁAGN4FGL J1900.4+0339?ìxï#—g¿ÕÕ° CÂMÀ8'_3l>À9í¦Ý@ø.åƘÖ@¢=ú	F?¼üÛ2k71?Õ,áàZH@IS.Ô)@TöÂ>©^?ïÿý{ÁA¿ÕbàõΤ¿ãCàµ7¿é)Ùîm¿ío¶;ÏÆ¿ïýŸÝÂUNASNone3FGL J1900.8+0337?µ:U"ŠÌ?À¥*.Û=\?íX¿U&3W?À¥*.Û=\?¨°
V<š?©ž˜›'¤?îtÿZW~0?©ž˜›'¤?À°e sÆ?°u¸£¾ï;?ëÓæ·ã`?°u¸£¾ï;?´lTû¥•`?›È•!é‹?íru`TS"?›È•!é‹?p£ï؛Z5?¨±É*ÈÃ?ïÞ¸ ‡"ã?¨±É*ÈÃ?xô•kÊý?†¯šN</?ïÎÕ?É*?†¯šN</?ˆã+âEª»?yHÔ¿éD?ïœsP"§Å?yHÔ¿éD?YÏòöÉ÷¹?LT¤;Å?ïóm=¬?LT¤;ÅPSR4FGL J1900.7+0426?ïµ5EJý¿§•TÝÊB{À7ù܄д¹À9‰W[0¨>@Û|_÷âO@tåÕ²Nœ?ÄÓ朁«?ÛpÇþ±Ì@@ õC
›Ê@"GÍÉ÷Û¿ïAhë{ä}?ï÷Œ"÷™)¿åœzŠ	ٞ¿ëj;=#¿ïÿöåv¿ïyöуóUNASNone2FGL J1901.1+0427?È}ìCNx"?Н€VÛ²?éà"ï,aø?Н€VÛ²?¤7uò|]?¥Šº®'$?î¾,ˆÊŠ?¥Šº®'$?Ï®xÆ1Êu?µk‡Õ'ñ?èaÎsc?µk‡Õ'ñ?¡~•84D˜?»ªÅÎÇG?îè¬a>×?»ªÅÎÇG?»'0Áá.?Ñ'•=ÇêC?쏾çÃÚ?Ñ'•=ÇêC?tÚ8.,?ƒ›ð†8é?ïÖKÇ?ƒ›ð†8é?¦×]	ölç?›^~²a?/)Ÿr?›^~²a?5ƒ"MDl?/ØgÈ^ƒl?ïýO «Ë?/ØgÈ^ƒlPSR4FGL J1900.9+0538?ÏeÓ¢®?ÞJ}ғ¶À8Kš2EÍÀ:%øÛH'@"ÞÏ®©@¤A"HG?ÈÞ½?ÚW<'W…ù@%B¯§ù@å3éf‹z?êàŒ1Ò
#¿à«µ?èM\¿è"³!*¿é"Ýr6~A¿îØú!ï"÷¿ïö[ ¸lUNASNone?Ê¿û˜'2?хü·Ì
?éPÛsY?хü·Ì
?°ÿ'ÒîŽ?²:Ue‡û)?íà
¥kE/?²:Ue‡û)?ØÁÖº?µüæˆEu?㟢ú@x?µüæˆEu?¾Gðwªd ?¢€Düé=?ì7ñ
³|?¢€Düé=?¥C›¼?¶9`?xw?î«ÆNGO?¶9`?xw?{sèäp£?ˆÊqÂ~Ùê?ïÉ/Õ8_?ˆÊqÂ~Ùê?¾j{®Ã'?®úè:§ËÕ?ì2°ŽJ'Ž?®úè:§ËÕ?b!Ü=j(?Rt{ƒØ1ó?ïíÞ$Ž|?Rt{ƒØ1óPSR4FGL J1901.1+0730¿ïÂí8ZÂø?ô9ÎÃG
À8Éw'ÕÀ:vnWÌp@J"á+~‰@%4åºÚ\?½ûÔ¢.=«?ÊBIP«éþ@©Ô#Ù?ø€''Þ@?ï¦~^Õ£`¿è¹Œ~($¿ãá"=‰ù>¿ä˜Õ^–¹?¿êœýýt¿ïb¾‰¬½UNASNone3FGL J1901.1+0728?Âׅ|EÂ?Æîã
"pñ?ëJ î¼P?Æîã
"pñ?½ÁiŠeÒ ?¼%&Ö«?ìGÒγE¬?¼%&Ö«?à35{Ú8h?¶­¼6 §µ?ߙ•K1?¶­¼6 §µ?Ԟӧ~Öí?°çµ½Xê?尖,@"‰?°çµ½Xê?‹¿&'#]è?Ž?D²Ž<?ï'g,xÉ?Ž?D²Ž<?"úx'Â!?˜j*Z
|J?ﯘÛ?˜j*Z
|J?Éâ³Fœz'?±Ý#	®û?é‡S.Xáv?±Ý#	®û?'[Ð–¯?}Q†ã8?ïu!#*?}Q†ã8MIXED4FGL J1901.2-7307?é
A©eÀ:"ŠT'À:Í*ô PmÀ<>é<o@FìËï?@7?Ŏ")uš¿¡¡ÛÇ*?Ü
ý¤[¢@F‹OSû*?ïù–Ys8Ý¿ë6¹ÀU›¿â¶ïö1J¿æ{þ¤Êû¿èíݾŒ˜¿ïÿ®XëTUNASNone?ïþ@˜ñ?"Ì9i‹ò2?+öu™eC:?"Ì9i‹ò2?ïôSüxÙR?[†ÜN›?WXÏŒ<?[†ÜN›?ïè
Ý_?ivÊRBCÒ?gòûî¢l?ivÊRBCÒ?ïû,c¶2×?*5!$
ÀV?CNp¼ÒÞ?*5!$
ÀV?ïý‹+AÍ*?2‹?®¡?3¦¥úb}r?2‹?®¡?ïÖa@ë5K?…mñ$cð?tÏ_~¶®n?…mñ$cð?ïÔ0¬<_?yÕUÿ[Ui?uçý/a0¸?yÕUÿ[Ui?ïân'–?]õœéÌ8?m鑩ã>?]õœéÌ8AGN4FGL J1901.5-2208?¹Pìiþ©òÀ([åÙäÀ:ä%hoUÀ<G‰ßrï@§Z
ã@u¦uJ/?Óãĵüý?×-KþSý@Ae%?ÿôæ³]¿ï—Jy Ö?ïüŃ,oË?œ0G¤í¿åß~ØÕ¿ã®ÈáÉ¿ïÿý¡UûŠUNASNone?ïÂwq%²?ˆ¦'rÖ-Á?~ÄGX‰Lþ?ˆ¦'rÖ-Á?ínœTÎ?¹‹F'7?´‹üM?¹‹F'7?î«ë¸V.?•¿?¢U ‰?¥AOEV"?•¿?¢U ‰?íͺ~I9¸?'Š-ÁÌl?±','<?'Š-ÁÌl?ïJ&ÈIbþ?–°	öãq‹?–»&úC<;?–°	öãq‹?äÍ۝ ~?ÑXÞþӅ#?ÖdHÄ¿ã?ÑXÞþӅ#?ísÅÊz?¥§{HdŒ‹?·taÓcýœ?¥§{HdŒ‹?åYBUSÞ?¸{NªßG?ÕùM{UXD?¸{NªßGAGN4FGL J1901.5-1112?Þ@î˜àJÀ;õ4v)À9ÇgŽ"'¡À;g2:å¯@Á"°Soi@"Ê<ϔ'?ŎºÈ"W?¿ÇñEÒó?ö®ÀWs"\@éz"¿ïh@[9â?ï{Ø»¿åæ8¨²f¿ìB­Yiþ¡¿Õaà89'¿ïù»þHoÛUNASNone?ïΙõ£Êd?¤Úú;:?x³Ex%õ?¤Úú;:?ï'lO«Ü4?§çtB$_?›v|?§çtB$_?ï
÷C1ǽ?'çá…#g?žA–Wld?'çá…#g?ﮜ¨ø?nÑ¿ìç¹Ö?"XûË98)?nÑ¿ìç¹Ö?îb×Ö?¯¨'t4Ƌ?®É߶Î!¥?¯¨'t4Ƌ?ê跜cùO?Çæù&ÎK?Ä]!ŽpÅ?Çæù&ÎK?êlzZAÈ?³ŠÛj{G??ÆN–øÞ?³ŠÛj{G??ìŔ÷ÉOÀ?ª¤ü–tÑ?¹ÓXAµ'?ª¤ü–tÑAGN4FGL J1901.8-0718¿èÈ\ù̓À}ŠÚ¹õZÀ:h'Β À<ª/@Kˆ{º
¨@$~d‰í?ËO¡¨Ü­•?ÜâÑ[|Óe@
&‹ýϤ@Áeý4ô~¿ïþ'A¶ƒµ?ïíjWŒ¯¿Ú
7`"j[¿âk8þNO¿ìÜʵ›X¿ïýÍáéOUNASNone?åÙ1£L\
?ɌC/T¬U?ÔMœ¹gGë?ɌC/T¬U?ãkďo'?Í^Í<«Ç?Ù)Ævá!²?Í^Í<«Ç?èì8‡}Y¿?°"_L?ÌOâ
™?°"_L?éée–ªm?£«¾ôÂÁ?ÈZi¥WŠM?£«¾ôÂÁ?Ëí\Î/?Ä¿c-e®?é¿(Ìt?Ä¿c-e®?Éòhíæ^?˦7&Wœ?éƒy¥Ä†h?˦7&Wœ?Ò³ÿ*?ÁDڀû¤7?æ¦?jùô?ÁDڀû¤7?ÓÏÉa2tò?¹ƒ£Ó5Dü?æOfŇ?¹ƒ£Ó5DüMIXED4FGL J1902.2+0448?çv/Äé©|¿Ë'^;õy"À8	Î^DIÀ9¥ÙUqK@+d²Lö@ãU9î8W?ÂJüèôJÀ?Ö–ä¦è@À7OøeØ@GNs*š?ïìPU'éT¿ã†áa¯H¿âÅîAÁn¿êX/ž‹q¿í]V½{öñ¿ïÿ§µ¼UNASNone?·pµ¯*Ï?ÄU)ù´È…?í±é æ?ÄU)ù´È…?¦©4ÖÇ.?¦ߗ?îŸul¤Õ?¦ߗ?ÅDsëgË?°¦²c*vë?ê®ã&
9?°¦²c*vë?¨…'²—ê?"•¤V0ð*?îw¦äŸ–"?"•¤V0ð*?ÀÑ
"Ñ?ӑ§º(?ëË 9=ZÌ?ӑ§º(?wF]ˆw'?"ȨÉûF?ïÑÏsSé?"ȨÉûF?¡ˆ_Ì£š?•3œGpmV?îçz‹?•3œGpmV?D8A­?9W-xçÚ»?ïúÿñÎu*?9W-xçÚ»PSR4FGL J1902.4-3417¿êÝ9#"éÀ0üÑc4'¿À;³*dW˜À< îؐ@¼´B½>å@elÖÂïÔ?ÐÙ¬SœŠ?ޔ¹ËhH¿@½í@?ü'Ð4`YÝ?ïÿÇ`|Aš¿Ûò¯àWîÿ¿ã³ú8?ân¿æ-ô/¿ïÿ‡4<G¯¿î^€SwvYUNASNone?íe}'%?ĵJâÁ?³ôÓyíµX?ĵJâÁ?⣂Ø{Æd?ÎÙyô¼?Ú¸úOs8?ÎÙyô¼?ëv:3Øt¡?¦~%*%?Â'0ž-}?¦~%*%?å«GÓ?®YoÉ@Å%?ÕáÄ©pYã?®YoÉ@Å%?íáZÖîÂ?¿Ñu=¦²?· õ*'dl?¿Ñu=¦²?ºCÅ<4¹›?Ãï-ÓU…¡?췇XyhÍ?Ãï-ÓU…¡?å°*L&A?¸GjM?ÕòŸ«g³?¸GjM?Àv?p'?¦á¥K#uî?ëâp<þãö?¦á¥K#uîMIXED4FGL J1902.5+0654¿ì1:ᎌ?åãÆxõµ#À8ߜ‡Š£]À:q=V¢¤@þ½QYº@#Ï!?À¦cAøD?ÎBðj‹º@x¼œÓà½@-ÙçÁ¿îܼßCòÉ?îÞgߍCË¿Þns恩¹¿ãª?K¿êŒ?ÿIvÁ¿îìÎÊÔUNASNone3FGL J1902.6+0655?ϋ?
åy?Í8š{@é?è8p<†¢?Í8š{@é?ٛ^aˆS?Í"Ëàyä?ã2PÏr»×?Í"Ëàyä?áš}¥ê'?¶ÑäØ'?ÜËý´*ü?¶ÑäØ'?ç³Ç1DÄ?®f¼xpóì?ИqÉvx?®f¼xpóì? Õ¹¤^Á?£¬MõX ?îò¤eƒ/?£¬MõX ?²`¿[R¿ž?½gp°ôÀ?í³èÚ`<?½gp°ôÀ?ŸB…¶Æ?²Òy€Ã?ëX/^'\Ž?²Òy€Ã?ÃÏÍ]@x?²ž»1¥Ü¡?ë>¨¯â?²ž»1¥Ü¡MIXED4FGL J1902.7-3246¿ãMž]<‹À0}»úëÄÀ:ÀÉÓIÀ<'oF	@dOÞ¾Š@ZR[íf ?à ð¥ïé2?Õ|8V1?øÞ<Pé'@^¬èÖC?ïü"ßphs¿ßÆí$ÒÈ¿è·ù1~'¿íÀ^à
AL¿¸¹÷2ú¿´¨¾û}å3UNASNone?íÄTÊ÷Õ?ŹýýœM~?±ÝY­öfÝ?ŹýýœM~?ïsÑ÷Œœ?žuÔv?'…Á
üÒ1?žuÔv?íºmdºó9? UÌʔ?²,"Ùºr·? UÌʔ?ï½3¯&k?o¦ll	?€³1=Ï>?o¦ll	?îšàÇ^+?²ÔLÄ"?¦QóŠù./?²ÔLÄ"?çm¨ÝâÒP?Ï?{Z5Î?Ñ$®D:[_?Ï?{Z5Î?é°K•æÂÓ?´9¿L?É>Ѩdô³?´9¿L?ëh9ÑC:N?¶ºðó$†?Â_ºóÊ?¶ºðó$†AGN4FGL J1903.5-0825¿²—èƒPpËÀüEßÞ!‰À:½……`ýÀ;!| dŽö@µIX8¦:@/ÂÝ_Â@zU_­å?ïÿûB«÷@
?h£Wˆ}?ý[îQ"ñ¿áô€oüè¿çF©½S2,¿ã‡Í¿;Ò¿î3Ÿ¿£n…¿ï¼ú\Rn¿ïif*×DUNASNone?æ+u£†Ê?Ò££c?Ó©¹þòl?Ò££c?Ú`¾x™?Ö0ØY6ÁÍ?âϠÞ>´?Ö0ØY6ÁÍ?é/E@.¡Ý?­"kAÅÝ?ËBêÿExŽ?­"kAÅÝ?ä¸Íó­%+?Ïñ
ÒY1R?֎d¥µ©?Ïñ
ÒY1R?äV͇ïÞ?Ó3Âûٜ?×Rdñò C?Ó3Âûٜ?¶Í-åìXƒ?ÇnN\"eU?í&ZBý¼À?ÇnN\"eU?à4²Èl?¾ßÅ^)½$?ߗ֚oÇ'?¾ßÅ^)½$?Á?•êëúB?ËFø~²?ë°…Eo?ËFø~²		MIXED4FGL J1904.0-5925¿çCf×ý"À8­f8C=lÀ:÷ªëÑtÒÀ<ibXº¬9@¸=Qo@ò
ú/§?Ðmn-E	?ÖüadôÌE@ð#̍ã@°StÇ'?ïû¯8gOš¿ÞEý$ÙSC¿â âiD¿éíŽ
t¿ïÿçáüú¿å¨<b5ÕUNASNone?ïŸù¥ø?ˆg­ë—Á?ˆº8wJ!?ˆg­ë—Á?ïöN6«?¤'Ò,ã+í?žþ!7ðøŸ?¤'Ò,ã+í?îU²ÆޘŸ?–6¸0°}?ª¤Ó^¨?–6¸0°}?îðv£S	p?¨¹§ð	? ø•Éó'?¨¹§ð	?<®²?£‡""P&?¥…¿ €—Ú?£‡""P&?éÿJhâ?É׀ËӎÄ?Ë´ÂÖ\v?É׀ËӎÄ?éMÎd?² IG—z?ÊÈÆo‡ïš?² IG—z?牶lÊ??¯M–6½Ë5?Ðíޓ&k'?¯M–6½Ë5AGN4FGL J1904.6-2713¿ï¼äMê;À-tG䛬À:
Gĺ¯"À;ãW4š@×K±Ú-3@±eÆ-v[?ÅuNá|Š?¹"{?òÎ|Iýz@¨_iX^¿ÕýŽá"¿Ã¿æ<æp–¿è—Ý6§[ú¿ãÿšr¦ç¿ïY=SG¥±¿ïËBôqV"UNASNone1FGL J1904.4-2725?ï얩z7T?`€Õk'Q?ciV`¬äŠ?`€Õk'Q?ïıj›ª@?…z¹¤á?}§JÏ—Õ?…z¹¤á?ï «'`~+?ƒ5L:Z·¹?‡Õr/I#?ƒ5L:Z·¹?ï¾í>dó'?eÌ_}⮉?€D°v9t?eÌ_}⮉?ïËÈT©6?z¾‡"U$?zt›´¯%C?z¾‡"U$?îLaa2¹ª?´«íȵ"?«9éëø~Z?´«íȵ"?î¾}Ʋà?œ?ØFÎQ¤?¤¸!Ý?œ?ØFÎQ¤?î1Ò&BÊ?—ž£¨È(?¬âݟ÷º^?—ž£¨È(AGN4FGL J1904.7+0615¿å"€è?;w¿·íêÿ'ÇÃÀ8ãöíôÀ9úio/bÄ@*VgjÈK@¶ÒàD²?ӕ`˼?áDpù…@¥Y³Ð|…@º>èÉ¿ë*: bK$¿o*8sö6¿æÉäð°ä¿í­Ôï°ýc¿íÛo'C狿¿¸à[ÊÖþUNASNone?ãÿyâ?Õ´[ÜõŽã?ÙÎ;ïè?Õ´[ÜõŽã?ËZšˆàlo?Çßb"Ò?é)Y]Çää?Çßb"Ò?à¿Èëã?µØhö©±?ހn)Ô9Ô?µØhö©±?à˜N4¸»À?¶Õ)"V?ÞÏc–Žˆ€?¶Õ)"V?Ëdlaä1Ô?ÎÉV¶°Î?é&äç†ó‹?ÎÉV¶°Î?ŠoÒ©cD?œü{6
Jo?ï•Â@ú£?œü{6
Jo?đ©Ÿ?­XQq}??êۺ՘<;?­XQq}??•?˜D¥Ž?ˆÕp…/F˜?ïV>ÍL?ˆÕp…/F˜
MIXED4FGL J1904.7-0708¿ïTꄇ}|À͔ÐÜüÆÀ9	wx¢À;'j¢5IŽ@)­RÞõ@3=??´ùÖ_—ý?×Òå XO¢@­H÷Q@xÀƒhTÓ?Ø÷}šµxr¿Ê!¯'Jq¾¿âHV°æ½9¿è6úh‹¿ë=¡ìNrT¿ïÿí )k3UNASNone3FGL J1904.7-0708?¹XßàOáj?ÀǀtQ?ìÔä:¼?ÀǀtQ?´1™ÚJþp?´ŒUj>?íyÌĶ 2?´ŒUj>?ՆX0
 ?µN*r×j?å<Óç·ùp?µN*r×j?Ó5]é¦^?°Ê˜©ªié?æe~Q,Ñ?°Ê˜©ªié?8¤L«]?….9'÷Ô?ïÁŽ·'&¥?….9'÷Ô?Š2]¥Âƒ?šSÉàòI?ï—6‹éhö?šSÉàòI?®Ò©kÚÖ?£Ñz&NÙ?îÒÕiBS?£Ñz&NÙ?
J  ¢?wEáٟÔ&?ï‹ÊÕbæ?wEáٟÔ&PSR4FGL J1905.2-5120?ïú™ŒŒŽÀ6ï6ÍòfºÀ:E£_9MÀ;ø(/Éò'@4êv*ÿˆ@-ô!¥l6?Èg$|a$ˆ?Ìj¹ºv^@ä ¦hµ@ÿ¬ãÎF¿½¶˜>6Ö¿âL¥)ð"R¿æR¿ >yb¿æü`£®ÆR¿é›r·­¿æ£Á`]öUNASNone?ïªp4#%Ó?"6?Z€:?…còú¦'[?"6?Z€:?ï×ïRˆ¸÷?}­Evj?tVÊÁ̕?}­Evj?ï™Èª˜d?'–·
´#?‰Õ]mƒ?'–·
´#?ïƹEër?^JÇ÷ށ?|£pz–ë?^JÇ÷ށ?îٝ,¦ý?¢$+ÁÑ?¢f.YÅô4?¢$+ÁÑ?ïD­Vœ?¥aW$Y'?—j\šS¶ˆ?¥aW$Y'?뙯+Q<‰?¯"1O
|?Á™CR»
Þ?¯"1O
|?í‹k²;ã?Ÿ¹íÜmÒâ?³¤¢ojÁÌ?Ÿ¹íÜmÒâAGN4FGL J1905.8+4942?¥ÖËÈ"À‹@2'0aǛ5À:õuD× À<Àêù¾:@à¼z-Ä@»|Bp½Ø?Î\^¥§ÄÖ?é§)¥÷ß@-9–ú'è@÷bõÑ¿à±`ôâk?µ¾ñlê9¿âi`Á¶Ä¿îª5]¯Þ¿É
ý«è¿Ô®)s–БUNASNone?ïÕAftb?¢Mnß?u_LúV3C?¢Mnß?ïx+ñës? $ñԍ?ú›ü›'«? $ñԍ?ì«Xܘ¥[?¥‰F³j;?º¥9:Õ$?¥‰F³j;?ï›tUšï¹?v4¨ÚNrƒ?‰"ꋅ¡î?v4¨ÚNrƒ?îr4áð0»?°¬•Ëöçg?¨Ü±â´ÂI?°¬•Ëöçg?é!`tèh?Íëå;ûÑ?Ë{æ~,^`?Íëå;ûÑ?å*ø¥~æK?¹ŸÌ¹–n?Õªµ3j?¹ŸÌ¹–n?ìUì—ݽ?°ä"1‹Ç?½P›A*?°ä"1‹ÇAGN4FGL J1906.0-1718?ïÐøƒcøÀ%æFÞ	À:ÙÒÛچÊÀ<Yíð3c@
æ®bœ@#5Y~ —?Ò߂\L(?ã›bý%Z-@x~a.ï@mMÅ×U?ïŒ3Ÿ¿£o?"2ޛù' ¿¼ÄfKäZ¿äô>‹$¿ïþ
A¢a¿¿ïcoqY	UNASNone?ìÛávÁÂ?¶­¤âç°?¹' ón
ð?¶­¤âç°?æñ(ª]?ÇfdZiû?ÒßÑ®«F?ÇfdZiû?ìÿÕÁF?¤ÂFŸ,É?¿ˆQõÒ?¤ÂFŸ,É?çu;´ó"ˆ?ª	lJ·ü_?ш–ºð?ª	lJ·ü_?äŸ÷÷6È?É4Ÿ'Dpü?ÖÁÆ'q?É4Ÿ'Dpü?Ð[ö«˜t«?Ì5,¿sl?çÒª3Ū?Ì5,¿sl?ã0Í}KÛ ?»}ïÑÖï2?ٞehIÀ?»}ïÑÖï2?Ô®Qü:èM?¸wG°ÔÚÉ?å¨×â‹Ù?¸wG°ÔÚÉMIXED4FGL J1906.1+1651?éxwHZ.@͉âlqBÀ:¦"Cƒ…À<x­"šB@ Gq=ÚÖü?þ¦öyn€ç?ÏjÜs­?ïmi?^º @\¾Fø@

 •L?ê}K…:¿î›éÕò|?åxUFƒr¿Ò&Æ0<‰¿ì³Éá`È¿ïÿÚ €UNASNone?Ñìi´?Ên)ö•ë\?ç	Ë|%üz?Ên)ö•ë\?Å!ýqÁt?ÃNÒ¬"5?귀£¢Ü?ÃNÒ¬"5?Ü9¬?tÆ7?²tŸ¾ÓŽ(?áã)àEœå?²tŸ¾ÓŽ(?Ç+¡6¤Šl?®HUMms?ê5²VÝe?®HUMms?¾½ÎI"a?Çë;ž‡¦?ì(^æ6͔?Çë;ž‡¦?"ý0Õ¦^P?£BàUcá[?ïXy`‹}?£BàUcá[?ÓáÒÚû0/?¼
5ÛP–?æ''gé?¼
5ÛP–?¡Ü©ët£X?œÎf–<5ô?îâ5a-8ë?œÎf–<5ôPSR4FGL J1906.4-2001¿æ¬»"ûÒÊÀ(VÑ|^ö0À:e-Ž¯À;»üߺ[@隆~‰É@D[Ëر?×µ?¿ˆ—?ãuf´iÿx@`†R•@ðÒæl?è9€õ]县ãE;©#zY¿à†Êßâ©-¿éoÿ¢.â¿íÈ1\™¿ïà'¢ sUNASNone?î0|S?¬ãHÓ9?¬ø?Ç_2g?¬ãHÓ9?ìÉ߂ºŽ?¹kL½
‹0?¹±ê+""?¹kL½
‹0?ê…FUÏÀG?©öµ}  ¼?Åêæ¨Àþã?©öµ}  ¼?ë1ãpÛ¾?¢Ô'bk;?Ã;Ìr<'	?¢Ô'bk;?ãøÓ½ú'?ʁ}Mޅ1?ØX"Îü?ʁ}Mޅ1?à0bµúÙ?Ðߜ–+ـ?ߟ:"ÌM?Ðߜ–+ـ?â6r?·´Ìß·?ۓ""Óÿ?·´Ìß·?ÞÁîÝmÙÍ?·É٘n=¤?àŸ'I?·É٘n=¤MIXED4FGL J1906.4-1757?ìïî¡¢–\À&™
þ`ÏÀ:_¦FPFiÀ<dÍ	2¯@MÐù^$@'ùºk¡9?ÈJŸ¶i3?Ô"Ãäƾ–@†ý<× ä?ûRŠ.A²?ïôÕ?/c¿àÞ1yÏϿܗ|=¾&—¿áDêÜ0¿íÖé¡éÜ¿ïÿÞ§À£ÊUNASNone?çª ßbjr?Çr7ïŸN~?Ы¾A;+?Çr7ïŸN~?åXn0µ?ÈãÿTš6?ÕáOÑ#ž–?ÈãÿTš6?ê½m¼Ï‡E?ªá‡k…?Å
IÁâì?ªá‡k…?èˆÇ¤ÄÅí?¥t,òƒ>?ÍÜálìèK?¥t,òƒ>?Ûú9J,'?̞þ[N?â'ãZéí?̞þ[N?ĎñêF8?ÆMv`."ç?êÜ~C…nr?ÆMv`."ç?àÁ¤*ŸÄ_?¾'O†?Þ|·ªÀwC?¾'O†?ѸõRZže?²¦÷â5zò?ç#…VÒ°Î?²¦÷â5zòMIXED4FGL J1906.9+0712¿î¼ÖÒ+©¿ÂöÈHٍ¥À7Ÿž;¿É¯À9Š*^x[[@ }øäWØÚ@˲5qÑÔ?µ®úS?ÉÙ×¢=×ý@A#=ó?õ· ¾œZ?í)#øÁG¿í*ÃQ#?Ùjä$'@¿ãýl§É¿êŒ<ït—'¿ì*úIݙ¤UNASNone?ydê¾	ól?•·ZZûŠa?ïÍ6*D³I?•·ZZûŠa?£U±@	½?¨\yœ†Û?îʤëÿd?¨\yœ†Û?ξF!L?±º—0?ènw¬à?±º—0?~%Þþ©ñÝ?o'ø‹ý"½?ïôB<eŒ?o'ø‹ý"½?•ïq5¤?Àˆ×@ð?ïP"v`ž??Àˆ×@ð?t÷¶ûž)?'´rkâç?ïÖԋ)Œ?'´rkâç?ÀzáG®?¬EmˆÉ±?ëúáG®{?¬EmˆÉ±?n¬ÆiHù?݆¾Æù4?ïÿŠqªà?݆¾Æù4PSR4FGL J1907.0+3556¿ÝÞŠ¹Nb@)A?À	oëÀ:؝@îÙÀ<^'ø»@Ò¨'Y.E@žº»RQ?ÐA°dmF?օ/IŒ;@$zü ¯?ÿ[Ô½0¿ïy‹Y?ïó}ü…!¿ä¶ùáØ͌¿è©H>]¿Ü2-d<?¡¿ïÿÿ" 5•UNASNone?ïçèCÃ?dÈú¥æ ?húºÝ
C?dÈú¥æ ?íåfdæ+?·z8q´ÃÚ?°ÔÏÔjÛ(?·z8q´ÃÚ?ï)½"–Ž^?ŒÒœA*ü?šÈOrUžG?ŒÒœA*ü?îÕæR1Ò?‡"²6äç¢?¢¡šÜ-ê?‡"²6äç¢?ïx`IŸcç?f	yoee?óöÃ|}:?f	yoee?ä½²Ó|i?ҘvÔr³|?×à"šY-?ҘvÔr³|?ìí\Ùí6?¦I8V_?¸•0)rÓ?¦I8V_?æ¤#ŒæǏ?¸œŸþ?Ò·¸æ2pã?¸œŸþAGN4FGL J1907.7-4037?¿ÃCÙk
7À4.gù
wÀ:€ž<–‰DÀ<*&i U
@šã	û'@,ý>" 
?ȵ&gó¯:?ÁŽŒ	äw?ñM¿¦sœ°@¤êÕeM¿ÜÌ~VG4¿Ã¬Ö!à$˜¿èìXþÉÊ¿æ­´©^3¿ïùà#kÀ?ïªóɐØ*UNASNone?ïû+tè?Eœ@	ÔÃÓ?Aû®í®Ð?Eœ@	ÔÃÓ?ïÛÈçò?'¸I¼óJ?r}›Œçó,?'¸I¼óJ?ï&rõ.Ú?­ÃÖº?Œ¶cSâUJ?­ÃÖº?ïìÚÚ誊?Q
[œ¡)?c%%Vµü?Q
[œ¡)?ïõý ÐI?Z3g'¶¨€?T¾ú\î?Z3g'¶¨€?ï+¾s²n?®íyŸç%?šˆ1ŽÙ§E?®íyŸç%?îz =³Ðä?œUk­¨8Q?¨Uü'V¦Ã?œUk­¨8Q?ï¦C‡O{?'sO•ÚìL?k7‰î¦?'sO•ÚìLAGN4FGL J1908.7+0812¿ÊôÀÇ/ÿÍ¿³÷
þp]áÀ8ì8¢Þ½À:™8JÊ)@'Sæ/@'D¦">?Àé+}1Y?ÙmucÚE@VºI<‰ô?ÿP­µ"¿£Ñte6¿çUá"oA¿äÕZXTU¿êޚú—
¿ìtVÿk/¤¿ïþ=RpæUNASNone?¥É€à™?¼'ü"?î£o¿39Ç?¼'ü"?¢àHԈ˜?¤3.ëû¼$?îÑþ»dù?¤3.ëû¼$?ÁèkÎ?¬ÄNj=	?ë…ýåxx?¬ÄNj=	?–¾~IiÒî?ƒÃZø'ÿ?ïJ
Ýì¸?ƒÃZø'ÿ?›Sÿ7l?Ã4²éGF?ï'e`==´?Ã4²éGF?tw)Ý=1?'Ï'Öž?ï׬J†?'Ï'Öž?§£«Ð¯®¥?ŸËßh»V?î…ÅBو6?ŸËßh»V?$AlÍÀo²?ßóø#šÚ?ïþ»é#?ßóø#šÚPSR4FGL J1908.8-0131¿á./èZ;ÀHðÄXŠÀ9,­m‹ô•À; mµ@æ@(¬ò'Ø?ÿè˜n#Ê?»KVët-?ÝÑÖÓ°@ ¸Óñ"<?ýÍBŸ¿á9|žCU¿ Î˜ÃŸ–M¿Úié=EÛ¬¿âÑeéŠs¿ï(¦G'þ¿ïþ#A"µUNASNone3FGL J1908.8-0130?n4ЏJ›e?€'Éõa«i?ïáË/¤ït?€'Éõa«i?£-û³6›?¥˜W¬è•{?îÍ D̖O?¥˜W¬è•{?§ç¦`*:?™Í‡ÖÐ;)?šDuŒ?™Í‡ÖÐ;)?ª2Z"
ۆ?'¬Þ5¸›?î\Ú]ÑcØ?'¬Þ5¸›?€
ÒÃ9+Â?¨_.Aú?ï¿Ô´Ö>™?¨_.Aú?z?3Q?…—ºbW?ïˁ™ÙÁŽ?…—ºbW?‰ŸµÓ¼?sYÏ%R?ò ?sYÏ%R?WŠýœM÷?I3w0¾s?ïô:}q?I3w0¾sPSR4FGL J1909.2+4646¿àƒ?íx5h@0.3ðÀ;7hWØ.*À<Ö{@›å،s–@UŽäÒ?ÍÉ4¼Ë!ý?ÙT%ò{@¼éåâGˆ@?UÑ{¿Ì?	U>K¿á͊,>Ll¿Õó"\¿áæ—䍳²¿ïìRnaÝk¿ïþß06)UNASNone?íëEc¿öƒ?¬ç_~,æ?°¥ÔãJ&e?¬ç_~,æ?ëx粬:?À¥æ»Ø«?˜a5O?À¥æ»Ø«?í"Øð<Ç?jOMFäÿ?³Y?ÉZÆ?jOMFäÿ?ìC­yua×?–[.Â
À®?½â"4TñI?–[.Â
À®?ëIX!Y»?¸Óƒò©°\?Âڟy¾™?¸Óƒò©°\?ØÀd+,s?ÏŒ+<Ö?ãŸÍêréÆ?ÏŒ+<Ö?æH€‹*Á?¹1WÒ)!?ÓoÚþéª~?¹1WÒ)!?ÝyÿÀE?´±u[û?ápC}Þ?´±u[ûMIXED4FGL J1910.1-4704¿©êß$é†À6ŠZ%"À:r·ÔCéÀ<F·`Sý®@8h§3`@J4CÔk'?Óà]7é{Y?åH-€Á±f@eöº «?öÔkçÛ¿èžç·4¿áw—±b
;¿æ¨¿aÕ2¿îì<fd¿ð?ðUNASNone?ïÛv¹£Wç?žòŸðã?rD£¦ ¢?žòŸðã?î˜þ›Ý¡?²ä…Zó@ª?¦pLpì?²ä…Zó@ª?ì:}Žª?§
œG;+d?¾+lŠ³?§
œG;+d?î£çòŠ?•-;lºl?¥ÏqŒ"^?•-;lºl?ïӖ9+´~?"q̧Š1k?v4ãeVM??"q̧Š1k?ã÷jÿ—F?ÓoùðúÝ	?Ø*ÑÙs?ÓoùðúÝ	?ê+ÆË^–A?­ªwŒyV ?ÇPä҅¦ü?­ªwŒyV ?ä,<P8ÿ?ĄŠÔ.ëÑ?ק‡_ýŽ?ĄŠÔ.ëÑAGN4FGL J1910.2+0904c?åQ
ìíÿw?5ïò<4üÀ8Dß-!¡À9òŽù,§(@!;êH³£@PwDŽ¥?ÀZyɹå?£¯a#}Õæ?ô0ÓÊ?ú$ÉâοïšG©â¼ù?ïÿd™ÝŒ8¿åµ)ã(Xå¿Ø•ýB`wº¿ëH¸ ÅÝſаh¾‡úUNASNone?àØËÞDn?Õ6''o?ÞNiàCw#?Õ6''o?åÓi0gžA?Ð4™ñiuv?ÔY-Ÿ0Ã}?Ð4™ñiuv?Þ@žD'ñ?¶ÇæM t?àö߰ݶˆ?¶ÇæM t?æ^\y?¹háÄ?Zj?ÒåCG
ÁÆ?¹háÄ?Zj?Ì‹µª$?Ñèp9×oÇ?èûÝ>'•w?Ñèp9×oÇ?Ôª.ð¶êk?ÓgÑ×3ê$?åªè‡¤ŠË?ÓgÑ×3ê$?ã^«ÅHҊ?¼Z¿1aTŒ?ÙB¨unZë?¼Z¿1aTŒ?ǧ°™Ì€ˆ?½$ŸmTRy?êٌßÞ?½$ŸmTRy$MIXED4FGL J1910.7-5320¿Õwoå¸xyÀ8>A_EàµÀ:~ùc<À<b
@@M…XÄè'@$$D'æÐ?Å6w
x~í?ُã¢Ò'€@•›Þwì?øöûú·Á£¿è›n»Ÿ}ß¿Å£œQÚ¾¿ä6žÂÎFJ¿çGú D®†¿îÒWPHí°?Ҕ«]¼HÆUNASNone3FGL J1911.1-5318?æÒyòª¤?É®
pq`?Ò[
ôª·?É®
pq`?ç…Ó
 å?ÉþçCàC?ÑÔôYê¾6?ÉþçCàC?çþ¾eśo?±Ý¦QÏ0?Ѓ4tÉ"?±Ý¦QÏ0?é¾l&ĺÛ?ª3§<é?ÉOdí–?ª3§<é?Ñ*¥eTÃ|?ÇÒƒÒvÊ?çj­MUžB?ÇÒƒÒvÊ?Ê*ø«fºc?̊Kˆ-z?éuAÕ&Qg?̊Kˆ-z?Ê$»ßrI|?µT™ˆ/lˆ?évÑ#m¡?µT™ˆ/lˆ?¼Ã:õä?ª–çFLtá?쇘¡]D?ª–çFLtáMIXED4FGL J1910.8+6300?ì^œ‹;ˆ@5Ø6¸ù±1À;eszK¹À<åyéÐé'@ .e2§?ÿ`UÆ2o?ÌC">™BÝ?ö©à8º\?ôˆ²ÁˆÌ@{2ü+µ?í‰?MóÔ¿ï韛†&?ïÄ÷u³¿åÎéõÒ¿ÖÍY$3ü¿ïÿÕ7ÕYcUNASNone?ïö£Í?œ "ݝ-?R¹ò`Jd?œ "ݝ-?ïòï²ïšÇ?_³)5ùú?Z šƒ¿1Ã?_³)5ùú?ïêªøÞðÞ?c%ŠÊeÀ?eUݶÊB?c%ŠÊeÀ?ïíùôÝQ?L€ñɊÆ?bç8}†Ô?L€ñɊÆ?ïýýÎ;P¨?*2ôä'K?0s[Ï4?*2ôä'K?ïż?"Dñê<v?}z"җ×?"Dñê<v?ïÝÌìØ0?vÖo,š}?q‰JVô?vÖo,š}?ïÛNñ»ÕÀ?gs€®?rX‡V°-?gs€®AGN4FGL J1911.1-3221?ÛS΃ÜÀ1ùÊâ°À:À1"öÂjÀ<BWڎV@í§¸Á'@Ñ>Eþ?ÑZ¨VÌ?Ԁo|Ä>@H÷}z"@ÙÙ7"@ê?é÷•ÞN)"?ãâ`b@fø¿àî`/뀿áñĞ*"¿îŸg~¿M³¿ïý"€U$öUNASNone?îþ@G]ë? vg(lÖy? þÞù½I? vg(lÖy?ïš‹‡F?¥ÙUSî?Ÿ®"F@?¥ÙUSî?í¬Sãð?ž‰
Ð?²`⦥\?ž‰
Ð?îqžâ??Š±ˆ ?¨æÙ{™Å?Š±ˆ ?í'SÏ,oí?°ç È€ð}?³ía‡æ[?°ç È€ð}?é1AƒÍ?ËbýŒnt
?Ë:ûéðÊ?ËbýŒnt
?ëa+Åfã?©…±9±B&?Â{Pêdsƒ?©…±9±B&?éoxXKo?´VԄ†tê?ÊBúÒD?´VԄ†têAGN4FGL J1911.3+1055?ã#P°­Ãƒ?ãgpQ¡³À99ˆ{¯¤À:•¦†è½@¡'Œ_t@íŒ_õ3?ÚBj?ÒËÊCZ°@r=äg?ú=k€3í¿ïõ¥¾Àðv?ïÿŽñ ¿çHÌAâx†¿çË,^WÏ¿í8="ßEu¿ïüÙçUNASNone?â"è©»êk?ÒXÐäçÿ6?Ûº.¬ˆ+*?ÒXÐäçÿ6?Ëö†Ëqê?É+A»ûÝö?é^M#…|?É+A»ûÝö?â‹Ëé߆?·ÁÍb&_?Úèh,AÚô?·ÁÍb&_?Ø*ÃÅ^Ñ?¶Î–ˆ6(?ãêžP·—?¶Î–ˆ6(?Íâ_]U#?Ëë$Ü£?è‡h(ª»w?Ëë$Ü£?•¥°ùðb?¥{òâݛ¬?ïRÓò…îí?¥{òâݛ¬?ÐÌ|ߓgÀ?µñþ"ßG?ç™Á6L ?µñþ"ßG?'Ðiçž?ˆwÉ'?ïq|°è+?ˆwÉ'MIXED4FGL J1911.4-4856¿íÄ\¯i ¿À7B«%(®À;5Ÿ>HÀÀ<óK¯Ri@vǕ«Mv?ÿ-gwžZ?Ðþ!ÃõÝ?èIè^9q@àýÜ9Q@ÊÇU> Ð?™cÿÙ¿y}? N>§?ÄHôe˜
M¿åÂ2᱿ïÿ;2G?߉ˆ>þB'UNASNone?éY)Ý(µ?Æ7"HF?ʛX‹‡],?Æ7"HF?ëÝIe_çW?À÷:GNè?ÀŠÚj€b¢?À÷:GNè?åÊU^VL"?³=Nð5-?ÔkUCSfÚ?³=Nð5-?êîG²à×5?§D4ȕ¢Â?ÄFá4|£.?§D4ȕ¢Â?ßî|§gÚÒ?ÏÔÄ¥X?àÁ¬L—?ÏÔÄ¥X?ÚýˆÎ½Š1?ÑM†XVÙ?â;˜¡:ç?ÑM†XVÙ?Êfuh??µ—²Iõ?éfb¥ð¼?µ—²Iõ?Ú0µqˆÐÁ?»dÊ@;À‡?âç¥G;— ?»dÊ@;À‡MIXED4FGL J1911.8+1447¿Ò[ôÀå@•@?ºÆà$À:-±4ÀÑíÀ;{miç@!A×0}÷'@˜¤§Ö?Âå9?¼®r¿—}4E?ÔïäÿÉy[@æÊ6Åcø?äE~Åý0¿á®å%‰&…¿çÅàŸgŽÚ¿è–•Ù¹¿¥¢¿76¿â›`^©UNASNone?ïÞ¸Jg_é?¦\Keœ Ž?p£Ú´ò³?¦\Keœ Ž?ƒ0¡ˆ?™¨Ò¥1…è?‰ß:¶ÕØ?™¨Ò¥1…è?¹¿vD?…<ç{Ÿ•?ˆUѝàÞÏ?…<ç{Ÿ•?ïí`¦3?PñÐó×?bŸYÂ N?PñÐó×?MÚ$?"u@̉h?‡],/£?"u@̉h?í6kÿØgá?ÀÐ÷ÝOZ?¶L ÎÍ|?ÀÐ÷ÝOZ?§+R"?™ûÿ©é©ð?¤uŠ·!Á?™ûÿ©é©ð?ïVï©#Wü?Þ坿?•"
ßœm?Þ坿AGN4FGL J1912.0+0927?î°7ÒnC¿Ìæ'Ú]"À8ÓbÀ:ÉîËû@Ÿ¼wjÏ@£ß¾AÏ?Ëṳ́ÞÇ ?Ô~ÊuÚw°@DG!ý€Ê?õiҩۆ#?ÑώH,¿|¿æ…¦2.Pu¿â¿-§Ù¿æÛWãä¿ïi§Šóä¿éb`¢­ŸUNASNone?ÎfÌgÍ?Ñ9À
ª@9?èyþfLæ
?Ñ9À
ª@9?µç/7Ô#?¸ÆÍ!Žù‹?íCd]«?¸ÆÍ!Žù‹?×­b3•?¶ŒžÃhäµ?ä)|Îæ51?¶ŒžÃhäµ?½,HÀ/§Û?¤3ÄùOÔØ?ìZvçú?¤3ÄùOÔØ?±Œ7!Ӆ?Á=†Å?íÎyŽ•ž?Á=†Å?dhö?•á®\"î?ï»ã™Ô
D?•á®\"î?º €œ%C?¨6(ë*‹?ì¾ëïì{X?¨6(ë*‹?`ž§éE*æ?S7"'³}d?ïïaXÚ]?S7"'³}dPSR4FGL J1912.2-3636?àƒƒæ‡'À3­Hˆ/À9û‰ø;æ`À;n'å".(@t9)ÂF6@§%?Tª?Ð^?ÜV?ϑ+6¯Æ@ëÅÃď@þü—À¦y?îÚ)'z¿ÕLÉè=ì¿éô§<‹Â¿éœhKBôq¿ëò`°
¿ÑŒ'Á)iUNASNone?ír™-@³'?ËÔi6­ï›?´k6•Œpq?ËÔi6­ï›?ì·ò껹?À`§rE?º@hª'J6?À`§rE?ì°.ÛN‰•?¥#7O"	?º~‰%‹³[?¥#7O"	?ía™‰9¶?—	y)—?·4ó5Ì?—	y)—?隕Éðf?ő…G–Ü??ɕ¨Ø?¶h?ő…G–Ü??×k)¤i+h?Ó¦å%ÍÞ´?äJk-ËjL?Ó¦å%ÍÞ´?ãJÁø¼?¶`J…™¹M?ØýÇj|ˆ?¶`J…™¹M?Ô'eÎÕª[?¶}Ýk"½?åìM•*Ó?¶}Ýk"½MIXED4FGL J1912.2+3621?Ö%Ç|xBÿ@'¬ì O*àÀ;˜Ø?ǖ,À<Ôe›eK´@(p¬@» ÒÞ_?Ü!3 ¾¼i?îbÑ¡GãÄ@
qU'Ù‹ø?þ:ñbÙ>?îAŸÝ€y¿ÓáP|ð§¿ÌËD˜¿ì·c^t)ž¿ïÿÞý¦ßR¿ï÷@s–VUNASNone?íŠÙ	=Ì?·kŒXúd?³©7¶'œ?·kŒXúd?ÞfWG‹¤?Î	žº?×[?àÌÔ\8:.?Î	žº?×[?ëۀ38‰?¤{…r?À'ÿ3Ü?¤{…r?×tƒ—q½?²"[Ugð½?äE¾4Gt"?²"[Ugð½?àžÂ ¹ð?Ñ6ß6ÿ?ÞÂ{Ó¾Œ ?Ñ6ß6ÿ?¸]I^e3?ÁY<@fç/?ìô\VÔ3Z?ÁY<@fç/?ä»ÎZ@"C?¹"Þ9Õ?ֈcK~Ùz?¹"Þ9Õ?¨W'µ•:Ê?• -S?îz†ä‹/t?• -SMIXED4FGL J1912.5+1320¿ïì²%+³?÷*ՖŸêÀ90‹µ«HÀ:ºðY|s@Ý$zØç@
¸·a+?ÇÅÿ©?ÔæÈ •¡½@àÆÜÈÃS?ýݹ\~0?é"Ë ¥<¿âõ:ªù›¿ç)ë‹Ô´ù¿ê^æ?d™Þ¿ïø~eET¿ïзþ^•7UNASNone?×	·Êî6?Ë­%'+èç?ä{$ˆä¸?Ë­%'+èç?ÃIè̇­‰?ÁM1¯??ë-…ÌÞž?ÁM1¯??äÚÀ"-™Á?¶eòô¬â?ÖJ~Ù¤Ì~?¶eòô¬â?Ø¡^EzÖ?®à¶#=ê?ã¯Pú]B•?®à¶#=ê?¹øƒÛ}zæ?µÿ;[úx?ìÀP£?µÿ;[úx?†1EkpÆ¥?"Y›Kâ?ï§:ê6À?"Y›Kâ?ÊLøi'FÂ?±pÐpÈ?élÁ囮O?±pÐpÈ?•¸ýÖD?~o4(A5×?ïW2?SŽ.?~o4(A5×MIXED4FGL J1912.7+4610¿Éë1¶JC4@/rÿÑÜ×À:Ï7Žâ†rÀ<¤¦Æ¨Æ]@W˜·Š @¬À½ÊÑ?Ŭï¢9Ñ2?×
;|Øæ@®0‡‡H^@0X,¼Ìz¿ÑŒž
²?ïcìÊì"¿á­˜‰Ï!;¿à—Lg"t¿ë!á1ßÈ¿ïÿý¡UûŠUNASNone3FGL J1912.7+4610?áç,Œ¥ë7?Éc"¡\S
?Ü1¦æ´)"?Éc"¡\S
?èqoõÂu—?Ȗl!ÄÔ?Î:@(ö)¤?Ȗl!ÄÔ?é)$!ـ?²uV³ç°?ˇ[oxš?²uV³ç°?ë·TW<Ÿ:?œßØD¢è?Á"®£
ƒ?œßØD¢è?Ȓ+ÀG?>"vo?éÛu:Oî;?>"vo?Ò¤ˆ^øwº?ÎUŠOhŒË?死ЃÄ#?ÎUŠOhŒË?ÍYþŽÏ?µsÐ>=ʳ?詏\L:?µsÐ>=ʳ?Ú63mÀ£?¹FÚÅ]íœ?â÷äæI¯?¹FÚÅ]íœMIXED4FGL J1912.7+0957?ï1Ð]ô¿Â¡«`ìSüÀ8™‰!|QŠÀ9ÿ¦sœ¯Ï@>Ž2Þ#·@æÕw–?É;΢ºÕ~?×B-'ð
@~Ò`Š"S@Œ1>fm¿îô‡%ùŽÍ?ïÐý¤-¿åȪ(]\¿çò—a°õ¿ïrÂ)ۛ?±	5ô–UNASNone?Ýsu¤X¸?՗ljƒÎÎ?áFE-Óð$?՗ljƒÎÎ?¸4ïçÀ)b?¹$½¸¶)?ìùbÃB¤?¹$½¸¶)?בÿ
P¹?¹L¡3åâR?ä7z×À#?¹L¡3åâR?ʑÝå›G;?±Pe˜{?é[ˆ†™.1?±Pe˜{?°`9×ù6ô?Ä ÐîM-¹?íóøÅE'Q?Ä ÐîM-¹?€ŽW׏kì?•ýݍz¬?ï½Æ Ÿ ?•ýݍz¬?³2êæs?¢Ø÷†ÿ»?íù®4äÂ?¢Ø÷†ÿ»?oRnèŽ?e›Ó È'P?ïàû­W^?e›Ó È'PPSR4FGL J1913.4-1526¿ëL"åB‡À'}ÚH¶R7À:¤$'–GÖÀ<ƒ¶85Ñs@¤¬é¶¹?ý+oðS?Ïd'œÒK?æðbžZÉz@‹&|k‹i@)WÅ8Ù»?ïéϘY(?ÒÝ¢] w¿»4J	Žt"¿àçÏAǺ¿ïùŒž^z_¿îTœÚ–¹ëUNASNone?Ô2"Hi?ÊvŠ¾èç?åæ¹6[Ër?ÊvŠ¾èç?Ëàâÿû3¤?Åýƒìç§ø?éÇ@3?Åýƒìç§ø?ؙk"ÐÃ?²$P©¿O?ã³J8n—ž?²$P©¿O?ÑÖ,¾âÌ?®«Dãp
•?çéû Žš?®«Dãp
•?¤µ"Ä͐F?­´ß7‹ò?î´­Ó|-<?­´ß7‹ò?¥:B¡e@?²oGÑï?î¬^['1|?²oGÑï?¸¡GŸ?¥l¤C?ìïË߉_\?¥l¤C?¨íC¸,$ù?™æo"I¿?îq+ÄTa?™æo"I¿PSR4FGL J1913.4-2652¿Ô7½lóÛÀ0c÷œ"/¥À:ºØ´5&À<cAfҜð@ž«¼±Ì–@œ':×lc?ÖiÀãàd¯?ïГ*êU@؍]b²?öô¾
'*:?ïîj}L¿Ö´¯àÄ¿ê†Jg,_¿ïõþ~pH¿èup¾®ý¿ï‰:;e0ÜUNASNone?êôñ4œP?Ê?ÕË	?Ä,;-Ž¿²?Ê?ÕË	?Ò&ªùLö?Ìå:®N?æ쪃Y…?Ìå:®N?è¨gÛº$?¯Á
Pög¦?Í^`'óo?¯Á
Pög¦?Çj\8Ô̏?°c½Á¹j½?ê%hñÊÌÜ?°c½Á¹j½?ä™U
o÷?Ò}gº#|Ý?ÖÍUå þ?Ò}gº#|Ý?ª[€§Ïþ?ºWrúë»?îZGõ•¡p?ºWrúë»?ák%AÐ?¸ß-!3Fø?Ý)ÿɵ|_?¸ß-!3Fø?½mãû?w\Æå$?ï¹
H`õl?w\Æå$MIXED4FGL J1913.5-0923¿Ò÷tøò¼îÀ"FQ	¿À:?þ@_ŠÀ;œò™åï´@OcJµ†@fnŽ›9?Æù¬¿;>Å?¡ç®ƒMî?Û⍩K@ϒ¾^¿Ð¸W_bf'¿æ ñ—‡q¿ìðŽ]{[@¿ÛÓ&Á½¥¿ë[Ë}lg\¿£f_Î@UNASNone?ïéEð5mÜ?tæýS?fºèγž?tæýS?ïÅæèä?†¥êü0ê8?}ôˆê&$?†¥êü0ê8?ïZpvÆÂ?ºÊ\S>Ì?"½ññ''À?ºÊ\S>Ì?ïïÒ¡U®;?Eƒ–.Ýú?`-^lxÍg?Eƒ–.Ýú?ï9òȒ‰
?tÃ
ž?˜Á¦ë÷k?tÃ
ž?îDÚê5­?³ÈÓZ§ã¬?§ë²R8Œ-?³ÈÓZ§ã¬?î¹f,s•?¢+Ånž>%?®diž­«?¢+Ånž>%?ïdÆ͞Ð?ƒb]å…ͬ?"g&QcÏý?ƒb]å…ͬAGN4FGL J1914.6-1157?î.ÀK£Ü,À%È%žÀ:Ë©·À;'gÞ5ªÝ@¼3ù¬©Â@ðRãÒ¢Ð?Ì)³ʅu?Öﺢþ)@Oá|‡:?ÿՐx2Áž?ï±åàïïg¿æYôhI¿â­[þX‹¿ëA«"ªO¿ð?ïû÷"IôUNASNone?ꘖԏ±0?ňý7k?ŝ¤­Á;A?ňý7k?äg›SÇÂ?Ð.?˜ò)Ô?×0ÉXp{à?Ð.?˜ò)Ô?ê^¹€-¦›?¬lÆäÁ»@?ƅÿIe"?¬lÆäÁ»@?êöþæ
Ǖ?§°m4zŸÈ?Ä$gÔáª?§°m4zŸÈ?ݐdå?Îôó8µH?át7ö͍x?Îôó8µH?³`Ç+\Æ?À5
w{¦X?í"ç«Ò×?À5
w{¦X?ÛÜÑóäO?º†
Ša\?â—
Ø}?º†
Ša\?Çï(6ªáë?µGÌïZ¶ó?ê5òUG…?µGÌïZ¶óMIXED4FGL J1914.7+1012c?èÕ×z¥¸Œ¿Ý3qÜç!7À8ÎFèòAÀ:6Ô­kÞu@OîýNIå@•ÁF†Í?ˬâa3¡˜?Ð+ØËސD@	]5<ø®Ó?â8èDU"$¿æ»/€÷e?ïõ8áÈÝT¿èÛª¶!¿æš¶š[`y¿æÄI,«¿ï—ªÝŽ¼UNASNone?Ûr´ @Ù?ÕóY'ê?âF¥ïú_"?ÕóY'ê?·ôy…æ?½i³«q;?ípÞÂ÷?½i³«q;?Þ½Z'À?¸R¦O'a?à¡wR¶Ÿþ?¸R¦O'a?ºˆøˆM¨?£)ç732?ì®àîöJþ?£)ç732?Û·Áź?ÔIïpCg'?ât$w#?ÔIïpCg'?ƒÑa'U?˜Ç… f³?ﳄº—ô‡?˜Ç… f³?×o%»)^?¸pmQAZ ?äHm"~kQ?¸pmQAZ ?`èËQhГ?Vz"M5Q–?ïï4¤øG?Vz"M5Q–8PSR4FGL J1916.8-3025?ÔÝaÆ&À2k‡	VÁÀ9ÀUWJi±À<2š†ÿ@ך¤["{?ü¡m¾I|K?¼((¾DÁ?Ñ|vžÏ@pÛjË?ùt(ì]`ٿ䇱°¿ã­¥àNß·¿Êf€Ä`˜¿Ü;Bö…¿êþþ"ZGõ¿æã"GþqUNASNone3FGL J1917.1-3024?à³+ª9
I?ʇ՛lFi?ޙ¨«ën?ʇ՛lFi?Ùà¾X,E?ÎwâB]{9?ã Ó¹iÝ?ÎwâB]{9?ã´dÿ'£µ?µJc"Ñ"?ؗ6ܸ—?µJc"Ñ"?â.Cp~S~?°éû7T'8?Û£yY?°éû7T'8?°M[xWÈ?·".[®?íÿVTux'?·".[®?¯¸Ä†ÿ¤?¼P­¾$úr?îw#€–F?¼P­¾$úr?ÂÝÜ˔á?¬iø[?ëH¿HÍÈ?¬iø[?º«È'C^?¥¬"Y€¬?쪆ûŸ?¥¬"Y€¬MIXED4FGL J1917.6+2609¿ëBÎeܱ@BèbTˆîÀ:\p\‰mÒÀ;ű܆~4@šš"P1F@§Jº8u'?ÅmbÁ_?œš±,ç?ÊL齞\?ñ'ç[ne¹?ïþ.H‰Ý¿æ»áWžL‡¿ëÄþÍ%¿èÄ$½Nªˆ¿ÒZaueݪ¿Û3Üȃ<UNASNone?ïB…@ú¤ª?¿äI'Õ'(?—¯WÞóœÄ?¿äI'Õ'(?ïÕPÔÙ·?­R"¨g>ˆ?œ¥Uáõ-2?­R"¨g>ˆ?îÉ)*VüÍ?šMýYŸ"
?£mmXØe0?šMýYŸ"
?ï§-Æ.Dƒ?p|ÈoÉP;?†4Žc@Ó@?p|ÈoÉP;?#úí?®ž,âra®?¦>êPµ2?®ž,âra®?èš$9MÝ?ÍȘÓÃX?͗oȋÓ?ÍȘÓÃX?í¥à@`Üþ?¢M?î•dû?²ÐýþBò‹?¢M?î•dû?ëŽ*["qP?±(•ž­íž?ÁÇV'î:Â?±(•ž­ížAGN4FGL J1917.6-3204?îY}ÔZúfÀ3*0"ÝzšÀ:CbzH›zÀ<*.y@-·qEèm@v"aKts?ÈS7_'·¨?о‰]aZ
@X/ž‹q?ý²-V?ï¹#!ÃM¿å]ñLÞÕä¿Þæg}'§ã¿çh¼LLí¿ê–`ÿõE¿ïÿ™s,ÛUNASNone?í¨ÏFqõ?²ƒß栁—?²¹…Ê¿2Y?²ƒß栁—?ì¸<Ñ^?¼u°Æ±Õ¦?º>Éu?¼u°Æ±Õ¦?íÒÁ&'…?Ÿ(·'ù¨}?±iöЪÔ?Ÿ(·'ù¨}?ìMª
ˆ£?œ(©ß]?¿5'¯«ºë?œ(©ß]?çéÌÏüØ?ůÕúóÒ?Ð,f`Oû?ůÕúóÒ?ÚÈ떼p?Ñ㳛DáÔ?âù›Š4¡È?Ñ㳛DáÔ?æ¿òÀ±%?µM‰Ìå#ð?Ҁ杷?µM‰Ìå#ð?ßBvb/?µTÐ.œ™«?à^ÄÎü|é?µTÐ.œ™«MIXED4FGL J1918.6-7813c¿ÛÆ7ÈÕWœÀ;æ·ª%ÙÀ:yl2š‡À<$aX"@ѧ*{ԍ@±ƒÞFqÔ?Ó@¼Þ˜&R?׈^2æ1?ûßFfìž#@Œ G2Ä?ï¾
'*:¿ÓíIå&_æ¿é´â_ܪ¿îú´|lb?з,<f¿ï¥c¯˜	UNASNone3FGL J1925.8-7826?ïóî\È
¤?^Ñóð­ž?X#FF¯h˜?^Ñóð­ž?ï걜öÏ?pƒR@¥È¸?eN€hˆ'?pƒR@¥È¸?ïWXv?'ǝ©lÍ?ŸÏÕÏ	*?'ǝ©lÍ?ïú(Š¸«-?;<»Áà?G]Ô£G"?;<»Áà?ï±äy;Ö?J^ÌRÏ<?ƒ†á¿ÐËl?J^ÌRÏ<?ï¡.C4]*?'L››î=?‡´o@§%x?'L››î=?êýÿ'ÐZT?²z?Ä´¾–²?²z?ï³ö·#d«?}â:ÑÆß^?ƒRCÝc?}â:ÑÆß^$AGN4FGL J1919.4+1313¿çd¡w´l"¿µàK¯«ÕÀ8YÂÅ+À9úád3†?@ïf£M!œ@w$ÄÛfÄ?Èڌ(õe?ÞUœŸ]}ß@žK¢•Áž?ÿQünûá7?ïï>ÜÇ?® ÃDõ1¿è'âôV¿íœáL¶'ø¿ïÿ¥!b%d?ïøDRëUNASNone?åm¾fyþì?Õ¥«®¢Ø?Õ$ƒ3(?Õ¥«®¢Ø?¶^'XH¹?µ¤Bˆŏ?í4-Õ-÷é?µ¤Bˆŏ?à›û‰'?¶ª̼	?ÞÈÄìûä?¶ª̼	?Ã46ÉÜ[?§ž"îogu?ë2òMºÈé?§ž"îogu?ᰍ!CÐ?י·Õ!¢?ܞå½x_Ò?י·Õ!¢?}˜Ù5©ð«?ˆÿ»Z¶9J?ïÄÎMwÏg?ˆÿ»Z¶9J?ÑÖ§ï·w?µI±8)Ž°?çÀ,$D?µI±8)Ž°?aÝ,ìG;~?U·u="ï?ïî"Ó¸Å?U·u="ïMIXED4FGL J1920.0-2622?åç}€ðf–À1"ÙºÀ:MV¿)vÀ<V'Tà@.ô®¾@I}<kÁ?Ç׫£Ì?Ò¡ä@Ü¿@
ª"Àā@4æv"1?ð?Ð'UØy©¿ãŽO¹{·¿åÀÌäIÁ¿ìˆ[NoÑ¿Ñ&w ÈÍUNASNone?ìr-w
?½þ29Qõ?¿Ìn"C˜?½þ29Qõ?ëZ-Ux­f?ÀÖf¾C?—JªJi?ÀÖf¾C?ìt,[ÂbT?¤'¼0½û?¼^!ìí\?¤'¼0½û?ë­'Ó®"Q?™ŠÏÉ£Äã?ÁK`±E²½?™ŠÏÉ£Äã?áQûèÄ$2?͏@ÃGE—?Ý\.w·?͏@ÃGE—?Ó]I…sâ?С	h×?æQ?[=F?С	h×?á¦Nâáü?¹v¶>x³0?ܳcò:<?¹v¶>x³0?Õ½}`Ë>O?´B#à?å!AOš`Ù?´B#àMIXED4FGL J1920.7+1334¿×qAJ;ý ¿È‰S¦EN"À9Êc&3À;vރ®uÊ@/ Ô ~%@Á›@bƟ?×ÓDç:·?ï•ÆÁ#@9Ë@D†r'&?ì®rn²e¿îZièÑæ?ÀË(²Ñ¤¿ê€ïHø—V¿ï÷Ú,0às¿ïÿüÉï£UNASNone?Ó3§šÁÀ]?˯;à^' ?æf,2ŸÒ?˯;à^' ?ÎUÎFR'?ÇêòŸÉH?èjŒnkv?ÇêòŸÉH?ä71F7áˆ?³µ?"¨°?בs<ñ?³µ?"¨°?ÄìónzÝ?¯Ýøã
þ?êÄÃ8¤aI?¯Ýøã
þ?²£æõÏE?ÀÉŗŠ†è?í«ƒ=¯‡?ÀÉŗŠ†è?–ú‡8<3?§ãצ%¶K?ïH/£ÓüŽ?§ãצ%¶K?ÏaM^ëü?³á	bÝÎZ?è'¬¨{E?³á	bÝÎZ?ªò۟æt?…&°âÄ,?ïz¨iYúŒ?…&°âÄ,MIXED4FGL J1922.4+1453c?ê¹æó…Z?­ºãôº/À8ɼHKÀ:%ç}R@ó¨9Dš9@©K£l3?ÐTa¡Z®!?ÚAœ¬s'@‰¤Òh@
‰ºr¿íxÚÂXՄ¿™¼S`'Õ;¿çJè3FS¿êÙ๨¿îª,ŽÔD¿ðUNASNone?á$çãK
ã?ÖwRj?ݶ09iê;?ÖwRj?Âàe»›¢?ÂêÂ|Íí?ëGæ'~?ÂêÂ|Íí?ܱxÓ¦ZÈ?µÖl2Ù?á§C–,Ҝ?µÖl2Ù?×2>×ȇ?¶"ô½Œ?äfàû"½?¶"ô½Œ?Ã{9  ö‰?ЇÛoOT?ë!1·÷Â^?ЇÛoOT?…¦hŸŒ?"% ·0à?ï©f_tH–?"% ·0à?Ál®Ý-›?©•ÁZÄ?â?ë¤ÔHŸ´™?©•ÁZÄ?â?"÷^¬ïÈá?zÄ'¥Ú?ï¬"…ù?zÄ'¥Ú8MIXED4FGL J1922.5-5233?é"'.ÃÀ9͋¤
âÀ:w¢'^<À<tñ´âg@ ÖQ…Ú@M œÃ?Ç6E¡ÊÀƒ?Ñ2%acr@@™'6@3{ùö{?îú÷íâÇ
¿Ê$ï"¸Ó¿áæüŽ[wö¿éC>n$Ì¿ét(%¸÷-¿ïý–-ÔN¡UNASNone?ïÙV;(¨ž?ÞžFÙ?sTâ'Yº?ÞžFÙ?ïä¿å*3'?sI_…ѯ˜?k@Ùìa:?sI_…ѯ˜?ïs7îaz¢?ˆ9ÇÊý?'™3ЫÃ?ˆ9ÇÊý?ïƎ۶°½?_ûB8"4é?|¸'2f~?_ûB8"4é?ïy<Ô
'?'?	o\Æ?ØewÍÖ?'?	o\Æ?ï¦*—`âÌ?•¼Üd¦e?†uZ èí?•¼Üd¦e?ìq6Š?§vÀ·Ò?¸ƒZ5R2­?§vÀ·Ò?îðb–!?‡$-uÕ­? ùßú¶î?‡$-uÕ­AGN4FGL J1922.7+1428c?ãYx[O¿ÊGBIP«êÀ89Ý3L]§À9†2Áô+¶@¥¿Ü#å@U>Lò?Ê&n©«àn?ÙÂÓº&×Û@ý8bGõ?ûvýz#Ý?ëˏJ‹>¿æ2Ï˄Î0¿â•ýÍö˜x¿éjª}ík©¿ïÿRáNd?ïÆ+B£éUNASNone?҇G™¾úÊ?Ӆ¾6m5Ÿ?æ¼\3 '›?Ӆ¾6m5Ÿ?²mŸ²è©?²5?u2rs?í²Ldê»?²5?u2rs?ÕewžG(^?·í2éye?åMD0ÜkÑ?·í2éye?½€õs_G?¨ôÙù^Ó?ìOáQ"W?¨ôÙù^Ó?Ò¨Ü,¼ ­?×N-TÌàï?櫑é¡ï©?×N-TÌàï?{»T쏺?†Å<,"•#?ïȉWñÈI?†Å<,"•#?±kòÊ}á.?¢·N@—Ú.?íҁ¦¢…j?¢·N@—Ú.?Trá
Ô¿¿?P~!%7¹?ïõƏµ®è?P~!%7¹4PSR4FGL J1924.3+1601c?éºÐÞªDã?ÉÎ81ʨÀ9uk¼ç|À:UùÖñý@ºE?Ð$›@8圧k?Ñ*YÛ=¨Ø?È.1× ì@IÄo0:?úٔ¾¾l7¿ÒñõNÌ?ï½Ë½ƒ-ǿ燊£\'¿é´ãÅ˜¿ãg†àzª¿ðUNASNone?åH^œ :?Ó‡PÛ~…?ÕïoBÇ¿Œ?Ó‡PÛ~…?ÔED,Õ¡?Ì[vÖ›Ÿ?åÝ]é•/}?Ì[vÖ›Ÿ?㞜ºØ¥ë?¸ !Í?ØÂƊN´)?¸ !Í?ã"KtÑå?·³bÖÂw'?Ù»i]Ô5?·³bÖÂw'?ܟ‡Ø"™‹?Ð÷½Å⑟?á°<½³;?Ð÷½Å⑟?¡twø¿VÞ?®Þ7¿p)?î踀‡r?®Þ7¿p)?ÛÏh@ŽÄ?¹ 5Á¿å?âK߸ý?¹ 5Á¿å?«Ó¢€¨Cò?¢F¢0)(?îBÅØø¡?¢F¢0)(8MIXED4FGL J1924.3+1628?àIP!f¾6?Úb<5:tÀ:k÷ÉЙ
À;'§WÈ=ò@#¾%7Çíj?ö·zU0³ý?Ñ£_ Ïmç?Æõa€ùd°?ì5J¿ì¿†?øߣ¡…KY?æt$'/¾¿ìW<'<ZÏ¿ßhŠãžJƒ¿âkÂ[YÂê¿Ù驼ÒXÓ?ȳùAI÷UNASNone?ïà÷˗ÝF?u]Q…ÐB?o4KFx?u]Q…ÐB?îèлÂ0?¬Ù
#´M?¡rôR'ü?¬Ù
#´M?ïv|Ë‹'?ŠÕkÖ¡?'0fžF[í?ŠÕkÖ¡?ïhÖ·Ëø€?åŠSðˆå?'å)Sü?åŠSðˆå?ï³
^RÆ¡?ƒy4ÒÎ!>?ƒ=he¯?ƒy4ÒÎ!>?é9O,§Ã?ÊÙ4í¦Ù?ËÂÃM`ö?ÊÙ4í¦Ù?íƒOf?¦ÔÖN´Kª?·7#窍w?¦ÔÖN´Kª?쾁_"?¯¨Ë^	a?º÷…;^?¯¨Ë^	aAGN4FGL J1924.8-1035¿Ûÿ#ârÀ(V>ò"{À9۰݂ývÀ;éü7ôc@™ÊM²o@Мe%õ?¯fõØ^Ñ?Þ{üOÇ>@>+ —ºœ@áù&Çêæ?ïé‹$£M¿ÓgÃþÇñœ¿Ý@`") ¿ß
)N­âý¿î'x_7H¿ïþ!†ù"UNASNone3FGL J1924.8-1034?‰ÊwÕF{?™g˜ŒØ?ï˜Ö f/'?™g˜ŒØ?¿‡'Ú+Á?¿pë$¦¨v?ì
¿äºˆ?¿pë$¦¨v?À`¥ºÂ½?¦ÛèY!-?ëÿ'֑OQ?¦ÛèY!-?Æ¡F/Óñô?¨v®¥Gâ=?êW®tƒ?¨v®¥Gâ=?'K åPÅÌ?ªW~üf@Ç?ï¶Ó|Gù?ªW~üf@Ç?›söÎA?ª'rœ×"?ï#"`/ü®?ª'rœ×"? ßß¼"7?'û"­Ãêr?îþèÀý?'û"­Ãêr?…@ã£gž?t\âó‹.?ïªüq;gÆ?t\âó‹.PSR4FGL J1925.3+1522c?&Z¿Ô"j…¯×ÊÀ8ۚ<VÈdÀ:@æp–@òµxrW‹@´ØŸhæs?Èñ7¥³®C?Ösâû¸G°@‹7T*?ÿ'Ú7Äg?ԊÿbvAÑ¿æË ýP£¿å·cyL8¿èàyAàJ-¿ð?ðUNASNone?ÒTђ?Ò$pE@¯?æÕ÷—6ùø?Ò$pE@¯?Ä•7ñD7?ÃBP/uìõ?êøš²®ò?ÃBP/uìõ?ߝ' E	?¸†ÙgS»?à|1>ïÝ|?¸†ÙgS»?Üã˜Q8?ºlÛ=±o?áõŽ3×?d?ºlÛ=±o?¿ A¦v?ÊͷȨœ?ìþ7Ë?Ñ?ÊͷȨœ?WÝäÊ<?‹™5ôî#ì?ﺠŒç7?‹™5ôî#ì?Áß½pÊ~¥?­/¬€|H?눣Í`W?­/¬€|H?‡Ú€+ÃÚ?UõùhÐ?ÿ'µH?UõùhÐ8PSR4FGL J1925.4+1616?áò¶'¼)?µä³HlUiÀ8+YhQ"2À:1°Ÿoœp@ @Ÿµ½f¨@ÈÌW\h?¶DË+­?¹=§UnòQ@Ž­…èÝ?ý´ý2p?®?ÅdÞ{öÆp?ïÊSá(¤d¿äV5@Ԇ€¿çÖÔÃ;S"¿å;$,/3¿à+Žž¾Ç{UNASNone?ÝÃí"to?Ô%RúÃ;?á	6EÈr?Ô%RúÃ;?ÙàËP©E?ώWòiÇ?ãšW¸+^?ώWòiÇ?Þ½²ŸòE¥?¼ÆÜÜ ?à¡&°Ý.?¼ÆÜÜ ?àBÿIXƒ?·TNœ"Lˆ?ßzmNù?·TNœ"Lˆ?ÒI–nc?Ó2•Às"?æøø[4ÈÎ?Ó2•Às"?²²"b.:©?½T$‰;p?í©­sž»Ë?½T$‰;p?Û¬²â&6‡?őüh,a?â)¦Žìä½?őüh,a?®'sF´õ_?¡Ô
õì=Ç?îØË¢o?¡Ô
õì=ÇMIXED4FGL J1926.4+1602?ä;ENÏØ¿Ïþ^Õ£`À8)çZÍÀ:*{¥t@^ŽÄÔ[@úv¾£>^?Âiž1Žm?Æ¥˜*ƒ·/@
‹}ý[àÑ?üÙ,|4ÙÑ?ïhD¢qYŠ¿áhÈv%÷¿åeŸ—	œ¿æñÑiÀ¿èEþFÂ\1¿àúsÅÊzUNASNone1FGL J1926.1+1601c?Õ°bêj9?ÒA™•	^p?å'ÎõŠÊä?ÒA™•	^p?Ð_с'fÊ?ÉDMÜEªs?çÐ?6̛?ÉDMÜEªs?ތnEáiE?» ¶È˜O?à¹ÈÝK^?» ¶È˜O?Ý·tTªk?³Oý@"?á$EÕªÊw?³Oý@"?»‰²±B­¥?Á‡fl¬·À?ìŽÉ©×ªK?Á‡fl¬·À?"~n)…2Ð?¥ƅa³Œ?ïdŽ¦ú?¥ƅa³Œ?բՍ:»"?¼`ÄÍ
E?å.•9b¢7?¼`ÄÍ
E?œ0…K1kX?ŠùiÝþÉ?ï{Õ}9U?ŠùiÝþÉPSR4FGL J1927.4+0253¿×'¶ú†!À·tî¿eÜÀ:nš»É.À;îjCk@5w>Cˆ@GEÙþäw?Ñk€'Í?å{h÷:^¡@tu½ò>v@~?NI¿Ù|½ÀÀO¿Ö†/¤³S)¿â2•"´¿ë u¡æv¿ïÿ{Ûèt?ïú!Dô&UNASNone?çÞjÌkm?Ç3º2§ƒM?ÐCï*g)&?Ç3º2§ƒM?êò߉Ïv?Å|ByTÞ1?Ä4ØÃâ)?Å|ByTÞ1?é¢ѧõI?®BƒñG?Éwà¹`*Ú?®BƒñG?íÉ]°Ï#?˜\ÃVTÁ?±µyõÒd?˜\ÃVTÁ?Ö;R¦ëçš?ÌÅ!3­?äâV¬Š3?ÌÅ!3­?Æô :z+?ÉOvYgi5?êB÷ñ`!u?ÉOvYgi5?ÎvX
ª"ñ?¹åÁû¸r£?èbiü•^Ä?¹åÁû¸r£?Ü­EŠ›q?¾âÁoJ?á©]:²rG?¾âÁoJMIXED4FGL J1929.0+1729¿è«=Ž‰xÿ¶Ÿ_´ÆqÀ8<ó˜:õÀ::&¨á5:@Tó®N@ ,Æ1¨?ººdë<#?ÕPâC5à@ôH!ˆ@+sxó†Ë?ï'ÞŸ]'ù¿Ö«³¢"NÚ¿ä¶b'$-¿è†"Ú8+¿îDl@šúÿïÎ$ É8ÄUNASNone?Ä rq°ã?É7W|‹
\?ê÷ãc½Ç?É7W|‹
\?¨2Ê,´hþ?¨3v\"¢?î|Ó]4¹p?¨3v\"¢?ÂléÜ{?®¡9ªNP?ë~¤Å¿á?®¡9ªNP?±ç¥%Ÿéî?œ6"U͂?íÃ[0…â?œ6"U͂?'X›kŽ•ñ?´%©Šaõ?ïu;$ˆq?´%©Šaõ?xþ K3ä?"9'ŽWí?ïÏÖØ&È?"9'ŽWí?¨¤-ºVN?£F$íï3?îu½$ŸWÛ?£F$íï3?N—»´?1e?Blð9Dz?ïøZCtI?Blð9DzPSR4FGL J1931.0+1754c¿ïàõèò>ĿӆoE],VÀ92ð¤BjÀ:‡4éد@ê''¸@_Ëâ˜@(öÎþÖ4?ÒÎBXõ»@
…凮¶@öˆþð?ïë@öjU?âA¦=—¿çuݜþ¨è¿çdœ,ý¿êϯj¼6}¿ïý "DsUNASNone?ÖfqT'9º?ӞSÂõ³v?äÌÇU¶ã#?ӞSÂõ³v?؛0h—]?ÒiQêл;?ã²wçË´R?ÒiQêл;?âHXÓxÁ?¶ó"a^ZL?ÛoOÈY~?¶ó"a^ZL?áÃ#fóA?ń
ª}í?Üy¹2ß~?ń
ª}í?½g¬PoGû?Ɔ
R‹µx?ìS
uò?Ɔ
R‹µx?°'"ž…«?¾Ý•-4|Æ?íï¯lX‡š?¾Ý•-4|Æ?Ò©ÕÈ/?o?·ØÊŠGC?æ«è`I?·ØÊŠGC?¨a
Ûç›%?®÷<ºß?îyï"jÁ?®÷<ºß8MIXED4FGL J1931.1+1656¿ã1 °}ûr¿éew•ÜvÀ8k§AøÈÔÀ:£ùnì@é'"§ŸÂ@蓂(cÌ?¸3žèãÙ¯?Øf¨@%‰ý@7Ý÷vÅ?ùõzÞm‰?ïÕM9Æö¿ÝËØü0Á¿ã£˜ ö/G¿é ÝDU¿ío³íöz¿ïàåõ"UNASNone3FGL J1931.1+1659?'%Ëÿ"?²GÁ‹_?ïvѧ–Ì$?²GÁ‹_?¤Û¹:þìu?©
"ÐÔeÀ?î²Dl&Õé?©
"ÐÔeÀ?²a7›ak?£½9C:	?í³ß™5Ï"?£½9C:	?‹[$»a›?v#àÜۂ?"¤9?v#àÜۂ?¸UÆÐYUN?ÐdPɾqã?ìõG&¦?ÐdPɾqã?uÔÿdF?'s(0í¨û?ïÔWå¼D?'s(0í¨û?Ž:ÇÁ&$?…-µ5z?·À?…-µ5z?#e¢¶¨I¥?ï-Åu:?ïþɦ—±?ï-Åu:PSR4FGL J1933.4-2711?ì€å¿Ñ«sÀ4§ã\[J©À:]«p_À<€»|Bq@k"§ïó˜@)ô?Ø]$?ÈÍfOÀ1´?ͪxúgº¤@à±5—''?øÓÁñQ'm?ïøU¦P¿äó~¢r[<¿ê_ý@²ø¿á'–
qH¿ïûÚ×Q‹
¿ï`낚y"UNASNone?îÈ>œ<‡?§Ižãé¢?£|=8'™?§Ižãé¢?é×öèejÏ?Æ$XNöˆ?È $^jTÄ?Æ$XNöˆ?íӁðŽ%¦? óâÍUð?±cðzDøT? óâÍUð?êÁ¶P+?¥*äH(2°?Äù&¿SßÈ?¥*äH(2°?è…˜áÏ?Æ?xMnž?ÍëõœyÈÄ?Æ?xMnž?Ìݯ¢pÐ?Ì©ÈA]ÿv?èȔ:×cÌ?Ì©ÈA]ÿv?è~á£0ò?¶—GÙå?Î{Ås<8?¶—GÙå?Ò½M½;ùð?´­ÇKâ	S?æ¡Y!b?´­ÇKâ	SMIXED4FGL J1934.2-1446?ä(_»ã«À0!BoçÀ:ײãâ"À<]՞,¦@KßS75@ôK+w}?ա‰?ïúºEዡ@©¿f²¼€?òJ̌¶b?ïûÂ^ôÆ¿âI†[Ï¿âp&¾°ªW¿ïþª_ºz»?ïÁ5Ø)!¿ÛèFۆ£ôUNASNone?ì«ë2éaX?ˋæÚ)Š?º ¦h´õ@?ˋæÚ)Š?å"Äåª6?Ò®uÞf¾?Ôöv5Þ«"?Ò®uÞf¾?ìÓW*‰A?¥›!'Qk'?¿yeF«µü?¥›!'Qk'?îaæáQ?¨¾ö‹½+þ?¯9፤ø?¨¾ö‹½+þ?늼ßh¥?ÇM¥|s:'?ÁÕƒ¾]k?ÇM¥|s:'?º6Úº1{?ÆqïÃ¥d?ì¹.¨¹Ñ?ÆqïÃ¥d?梢`cÝ?´°ùQå(?Òº»>ý8G?´°ùQå(?Ú¯ž+'Bn?ÒäÁ÷—âÆ?â¨0ê>ÞÉ?ÒäÁ÷—âÆMIXED4FGL J1934.2+1036¿ïŸÔì½Àdf±æÀ9ê¡/"À;q¨žð@u+'SO@êÓ²š?Î8×!qÍ?̪'».å?ûìÓi©@Ú!« §¿ç¼uÁù	A¿âŠI{õ¿ç«Úy]¹ï¿ç!¯}0­G¿ï÷ä]b0Í?ï(ڟsMUUNASNone?ï½:†lHÜ?€ª~7-?€±^W/Y?€ª~7-?ï‡!å¥X?•?ÁôÈ ?Ž?w|GÖ?•?ÁôÈ ?îøÜ%7ûx?'Œ'­§q? r=«¤aˆ?'Œ'­§q?ï¬ñÁŠ	À?pqÌÒºx?"Ï í,?pqÌÒºx?îYªàW²Þ?¨'ÎތB?ªeQû`¹?¨'ÎތB?êgŒaxk?ÉßüÄ%"?ÆaÏÞzT?ÉßüÄ%"?æVn†›e?·ÝÏ#NÐ?ÓSÑ"òÉ6?·ÝÏ#NÐ?ë—4*ÂE?°P¶puü?Á£/Wäöî?°P¶puüAGN4FGL J1935.0-0553?ØOn&oÀ(¾Ÿà·öÀ:(òvªHÀ;­Ëwb7-@^R 3Q;@Ç>
&Ê?ÌVïûÐñJ?ÉÀœþ('?û)¢á@ø@ÊQŠŒ5ƒ¿åu¿äF¼¿á"՝U漿êú©]\¿âSÓ¡Ó#ÿ¿ïÿÿ" 5•?ïâÞA>c¾UNASNone?ï´º­ne?'¼*o"?'ÑT²'¯?'¼*o"?ï´È'oj?ŒI׸®Ê¾?'Íúè³n?ŒI׸®Ê¾?ï2žp?½R±RÉ?™¿,?ýr?½R±RÉ?ïÕÅd"¿H?aWÐM—+æ?uM֓M?aWÐM—+æ?î}»ä{?®s€AŽ'¼?¨.ÿ"eÑU?®s€AŽ'¼?ìútqb?¿Æe!e?¸,_"tï@?¿Æe!e?êSxòýZ?±±˜†!¬H?Ʋ4
•ý?±±˜†!¬H?픜®»h?¤!÷ˆ£'E?³[‹è<?¤!÷ˆ£'EAGN4FGL J1936.6+1921?ÎôÔÞi,i¿è°IáÀ9"+zMÞÀ:µ®Ò­@Ù£‰²pÖ@€"Þ?ÉSàQäÏ"?Ì%=§*{Õ@àÌ¡-â'@Òÿ–ÎŽ?ٜ߯}‡?ïùRژg¿çÝgNòr¿æj}2…
¿ïþ;·f3?ï±<î×íUNASNone?éïm.½¾Î?ÅÙ{.–ä?ÈBKE	È?ÅÙ{.–ä?áLé2:â?Ð{]s΃Ü?Ýf-›ïŠ<?Ð{]s΃Ü?畷Kӊy?¶1ñ¥md?ÐԑhXë?¶1ñ¥md?ç'5!þ` ?°°&~z÷p?Ðݕ¼?¿?°°&~z÷p?ÔÍú*9J¶?̙.¸'Æw?å™êãZ¥?̙.¸'Æw?¯Ñí'÷
y?ºùâÉR2Â?îá&©•™?ºùâÉR2Â?Ôiå?»/òÃÎÿ?åË~öwx?»/òÃÎÿ?»ß	a
ó?¬pi™}"I?ì"ÓÞA?¬pi™}"IMIXED4FGL J1937.1-0444¿é5K±Ÿ†À(¥îÇÉXÀ:§
ûÅ<À;בÕùµ@ŽÊɽMÔ@Ñò¦{)l?ʞ#×u;?x	‰k¤ï?´!ˆ¬6@5™ ûb·?ïO5'‰ ¿ì¿ôÕ÷¿âѱkë¿âLERðgÝ¿ß=W´¿ï÷ˆ—é–1UNASNone?ïïŠ
¾¿?eÍRÁ«?`uõäÁà³?eÍRÁ«?ïÊÍ·‹û?…5¸AL?zû™ÛjR?…5¸AL?ïž"³ðC0?"øçX,?ˆwRö0Ä$?"øçX,?ïå‡Êí‹?PZ†páVT?jx5ÐUE<?PZ†páVT?ï´»ð Ud?ƒŠõòtùê?'ÑΣ´ù?ƒŠõòtùê?î¿ç8ÞÃÅ?­Í^R|ÁË?¤ŒmÈ@²?­Í^R|ÁË?oðþ°?žQJHÄ,$?¦‰ƒÉø?žQJHÄ,$?ïS9jɑ?"êÏÿø—X?•œ8Ò¦Í×?"êÏÿø—XAGN4FGL J1939.7-1242¿³ä77ÿ¿¡À0`À½ÊÑJÀ:OL{ٕ2À;äñ"«=@ã7sá%@÷>^‡?Ï"/)ä*?ԏ=?{•ø@VÿëJ?òoðJÖ=?ïá·uL³7¿ã¬u:'Ä¿éb†ÝÕ2Í¿åãÈý4s¥¿ïÿÕ} i¿ïä×»=XPUNASNone?ì¿ëPך?Á[U¤³d?º¥yC/L?Á[U¤³d?⠆Ð5¯\?Íãü"i¦&?Ú¾ò_"¡H?Íãü"i¦&?ìæ*Ý¢Í?¢&e–óý?¸Î¯—[?¢&e–óý?åRÙ?»›'?±¡añÙîì?ÕZM€ˆÈÞ?±¡añÙîì?éŽ{fä̯?Åð©7"·z?ÉÆdlÍD?Åð©7"·z?¹Ÿ¦s?ÂÁ}C!½À?ìÌn1ž?ÂÁ}C!½À?åÿ±
T@?¸¹Ž_Ø?ԝñåW€?¸¹Ž_Ø?½NÍX
O?¤ƒ<è÷L?ìV&Tþ_?¤ƒ<è÷LMIXED4FGL J1940.2-2511¿à¸û-՝£À5[«!ZÀ:61•¤A"À</Æ|P³w@Œ8ê8C@ZمAóÀ?¿ŒãÓ¤'V?ЀhûÂÄ@·»Ã
@%£fÌè¦?ïщàiÝ¿»Ž>Wå«¿ãi–!!Ë¿æö.Åæ(¾¿æåP¡F6¿ïÿÿ" 5•UNASNone?ï
ôª¹?¦…µM^•}?žA|Âvè?¦…µM^•}?íæ›î¯ø?´Z-·¸?°Ë Žx¥Ä?´Z-·¸?ï#;gùÓ/?'‡Á‹_?›˜"¤Ò?'‡Á‹_?íå$Èiï;?eçü®/á?°Öٻԟ-?eçü®/á?ë
ò!p?½r:@SéG?ó÷Ô7z@?½r:@SéG?àÿ>™:E™?Ñ>qi= 
?Þ'Í‹tÏ?Ñ>qi= 
?éܲjöÃì?±y²†Ù??ȍ6T$ðO?±y²†Ù??ã_z&6Ën?´ADW*±?ÙA³'i$?´ADW*±AGN4FGL J1943.9+2841?͛B­	õ@!‹zՉÀ:—{!ŽÀ;ú¨(÷@UÕ¢ß="?ÿ'þtå…*?ÒM£!Ø?á÷Ix@æþ*¼l?û?P"]?è¤zÏ)¿éS-Ú-Þ`¿Âë·sŸ4
¿å0>·ç¿ïûêAQÙç¿Þ»k›¯svUNASNone?îŸÃ¾¢?§n§bæò@?¦Ï~"Ý?§n§bæò@?㷕Ì
<Ý?Îœ8¡˜?ؐÔgå†F?Îœ8¡˜?ìHñ°d•?¤¦‰ðmá'?½¼r|ÛY?¤¦‰ðmá'?è\ʇçÚ3?¥iGՑ?ΌÕà`—3?¥iGՑ?ê£(¾æV?À\T´ã!"?Ås]gî§?À\T´ã!"?»×V"»?Á͖'9d6?ì…<
ˆ?Á͖'9d6?䕿Ž#Â?»'iÂ?ÖԀãó¸}?»'iÂ?҂¯	éÊ?²¾…Û»kë?澨{x‹?²¾…Û»kë	MIXED4FGL J1944.8+4301?Ã
Á†êâ¯@"ˆ^	}À:ߝcRµ¯À<®nƒkYë@š7›Í¦?ûewS´?вï«ôæ?ÝßÉÿ'ò¶@
°Ð?Hl?ð\^š/A¿î'@"ªt?ïý%Ÿ÷¬Ÿ¿Ð×L¶8Œ¿·ByLG+c¿ë4rÞn೿ïÿþ½à ¿UNASNone3FGL J1944.8+4300?ìsõò¤¼|?½>ÖnP'?¼`PjÚ?½>ÖnP'?Ø=2œE¬™?Ì"U…?ãáf±Ý)´?Ì"U…?ëX¦ªwÛ?©÷>€èIŠ?g'V •?©÷>€èIŠ?à!ÖAÉ+¶?±9	þœØ²?ß¼S|m¨"?±9	þœØ²?å²u¢]Q?Ç5øNI¨Ú?Õò›»E]?Ç5øNI¨Ú?³ÆÅG"ò?»Ëçù½µr?í‡'WŽò?»Ëçù½µr?ß/A-"/D?ÀI¤¨…4?àh_i5è^?ÀI¤¨…4?½Ù®…¨»?«ôÞ{ÛI'?ìDÜ*/Jé?«ôÞ{ÛI'MIXED4FGL J1946.5-1527?îÕ}J1IÀ3ªCåÀ:­;qÆÀ<2©ˆúåå@+QœU@MdQ¹08?ÌZÂl½?ÖÂ{»[@û͆00I@$_6œIL?å*zAå}ž¿ØôKâ»'¿ÒЖ‰B¿ä¶ÌR֒¿íÈi[
lпïÚ/÷>_UNASNone?êU÷˜}e?Áž2Ìl:ø?Æ« !ž
m?Áž2Ìl:ø?êTŠ|"îË?ÁXˆ2Ð ?Æ­ÖtDÔ?ÁXˆ2Ð ?ëºCä'?¦3Ó¤ÔÌ{?Ášñˆmø?¦3Ó¤ÔÌ{?ë"Œ™ßm?›ñf7¬?Á¯á͘'K?›ñf7¬?Û·)JYÈý?ʘæÞØ?â$kZÓ'?ʘæÞØ?Ò̋D¨aÅ?Í=ÚãÞ-À?智]«Ï?Í=ÚãÞ-À?à0eÙ¬6Þ?½ÁFöx[ ?ߟ4L§'D?½ÁFöx[ ?Ùc3''Q?µ¥Q]?ãNf7l}Ø?µ¥Q]MIXED4FGL J1947.0+0031¿á@–wj¡À(2¦Òg@À;KÍ]ìÀ<±
À¾¢@Ͷ˃¡‹?þˆKBôqW?ѧ+='¨?ãŽYM= @º2nU"@ìé‰ò?ïõ-¿‰?ïý¤ Y?Ùς‰²›É¿Û®âÛ¬ä¿ê¬í3t¡"¿ïý4©Tø€UNASNone?驺hòî?Åf†œ"?ÉY\7äH?Åf†œ"?æ¦l87~ò?̦y¯w!?Ò³''?̦y¯w!?é¤ûï¯P?°7°&–H?Él"ABÀ?°7°&–H?åéøi…?²ÎÓ}L#H?Ô-òÁ,õ?²ÎÓ}L#H?âÉŸ¹æŽ?϶0y֖á?ÚmúÀŒ2å?϶0y֖á?Öøæ¬Ø÷º?ÒŬ¥˜‰?䃌©""#?ÒŬ¥˜‰?×Û,(yŠ?»
»Ç.Ž?äiëðÃ;?»
»Ç.Ž?֙ó«!Æ?Á‡ˆeûÖ?ä³*o÷?Á‡ˆeûÖMIXED4FGL J1947.1+1729¿Ã˜•£íxÀËEˆ MÀ:~]yWÚ²À;ïpx8 @YYJt@ˆÞ{Jùù?Ò¢É4<?à®
>¬ãù@&Á» ÒÞ@ªåq^?ëgÇÅ&^?ïÍýº¿Üê¥OÛ5¿ßŽØ'?Ù¿íÃÌ"'áÇ¿ïéý"ë´ïUNASNone?ï5nŽup'?™°òÕÖI?™R.4Á‰À?™°òÕÖI?ìˆëˆÕ?¾/²µp‡?»¸£—k¹Y?¾/²µp‡?ìkÁ''ë?£ë°dLµÚ?¼¡÷>Ãè«?£ë°dLµÚ?ëmµýZy?¢z²ã<†á?ÂI(¦–?¢z²ã<†á?ësNØ;|?¹Ï˜¦vï?Â2ğ³?¹Ï˜¦vï?ä~Öî|!?Ò™\L?×R#Ó¾?Ò™\L?è%"˜ofÚ?±{ç7IQß?ÏiížBd˜?±{ç7IQß?áPòSøƒ=?ÀFz¶ˆt?Ý^Xù‡?ÀFz¶ˆtAGN4FGL J1947.6-1121¿é­PÚ|Ò}À1'à°«À:&whiÏÀ;ñ"ï¾i]@LAô—2@÷T°[|þ?Àò1uÃÑ|?ËÚ\S=@áÝBeÖ@îa§ºÅ?îúA¯Í¸…¿äÅïbùÊ¿ä˜zJHùn¿ä¶"¡¸!¿í6A
çI¿ïÿï0l¯UNASNone3FGL J1947.4-1121?éG€ËӎÄ?IJv2>õ?ÊáüбÄð?IJv2>õ?êˆ	æÖÑ?Á;ù¤àäK?ÅßØd§ì»?Á;ù¤àäK?í5•|î,?£çj~eâ?¶STØzG?£çj~eâ?ëµTÑúšL?šp]ùm?Á*¬¸–Ñ?šp]ùm?Öè¥Ì¾ñ(?ÊDøžsi?䋭 ‡l?ÊDøžsi?ÑÌ»µMTG?Ìõ€ø/s'?ç¢%YUÝ?Ìõ€ø/s'?àÍÝ¢¡ÄÐ?¼wò¢iU?ÞdDº¼v`?¼wò¢iU?Ö –Sû?²CjAg?䯴Öw÷?²CjAgMIXED4FGL J1948.0-2845?ä¤Ñ{ª"À87÷ß (À:Âôí}F}À<'øxLAø@õÉ¬²@ÝӅM²:?Ҋä?Z2ü?ÆÍyÛc='?öéjâÌéR@vMP¦?ïó÷H¡Y¿èM!@—tÑ¿Þwgà¹é›¿åá*È*§¿ð¿ïýl§ÉEUNASNone?ïô€"­³? ߗ[¥
?Œ'àK? ߗ[¥
?ﻫf.Þ?Š«<?‡"?;©ãäx?Š«<?‡"?î^uRùˆ?šK·A'ñ?ªx§`ˀ?šK·A'ñ?ïjÞN?pPê&B•—?Œ :(¸"?pPê&B•—?îòàu	±?¦ue–^†? Ñÿüé?¦ue–^†?îIk?$iR?±íyL"z˜?«iL•QÞ?±íyL"z˜?ìwÂÀôU?ª-®A¤î•?¼Aéø_UY?ª-®A¤î•?í•Cµ¦.l?›_ñ|.¥?³UâQ"² ?›_ñ|.¥AGN4FGL J1948.1+2511?ÕT÷Ëu.¿ÆÆ»üXÀ: !}(IËÀ;ÎôX,@ŸR–$ð@L¦¼—Ëc?Õ¶?!}ÿ	?ïý½À•[ò@Ö|^p@'ܾ²X¿îêÎà£Cg?ïƒP˜È¹¿ÂTR½'M¿îAŸÀäa¿åË@¥â}8¿ïþ½_ÇeÛUNASNone?êÝaŠ…?É{—éɳ?Ċ{õÕëÁ?É{—éɳ?ã¢aÇο?Îì¿9?ÙÖ»<pb'?Îì¿9?èfìÐ>±?±ÉU³ù‡º?ÎdL¿»>?±ÉU³ù‡º?äºÊ¶òðÎ?µÀ–Ox"Y?֊j'd?µÀ–Ox"Y?â[/ä*¦?ÐIÅÀWã0?ÛI¡7ª´?ÐIÅÀWã0?Æ4q®Êa?Ênˆ`ƒšÌ?êrã¸TMh?Ênˆ`ƒšÌ?â†Ã"K{Ì?»%'E•
"?Úòy»ih?»%'E•
"?ÄCõ€Ó­š?°¸Ä#á,?êïŸË™?°¸Ä#á,MIXED4FGL J1948.9+3414?í‡óç˜Õú@ùÉÕ¡‡¥À:Œ%ÿnÀ<d._ŽÛÐ@€Pþ .‰@'ƒ$ã?Ì)FNm÷?ã$"¯&ɘ@4·|Ùor@*¥"8äù¿ïþ1ɦ§Ÿ?ïÚÚ¬‰`f¿Ï®öxçù¿á©=¦~¯¿ïÿ›‹â ò?×Fë¡Ï4UNASNone?ãiç\?ɲ	ýÚ·?Ù-ÚÄ1GÌ?ɲ	ýÚ·?ã±œ?ÏêE®ŠíY?ÙçàþÇà?ÏêE®ŠíY?âHŽ-]d?´3$öë•v?Ûoúã¥E8?´3$öë•v?龃Û8"?¥ õ&´Ôñ?Éð"ëµ?¥ õ&´Ôñ?œ¥p´À?Á
»Ä*«"?ê›;£ÒÐ?Á
»Ä*«"?¼Ï41ée?Ägtr1‰?ìfùyÂÓ?Ägtr1‰?¼tÍÔ¬¯?¨ø[ÒÖÕy?ìqfEj~Š?¨ø[ÒÖÕy?шõwb?¶"©Òe¬Ç?ç;…vÄNñ?¶"©Òe¬ÇMIXED4FGL J1949.2-1453?ë
Ôæ±À3c 1ί%À:9ìTRÀ< 5)­x@584¤ÍT@º®ƒ?Â-æ˜$ú`?Ïç™Â3k½@
®Æ±@£'ôf™½¿çXJCðñ¿Ö·_þs¿ã
çŸïõ¿ã9>Js¿ï¾'€p}Á¿ïûúëÄ	UNASNone3FGL J1949.5-1454?ê%ôG~Þq?À­l…]?Çh.â†;?À­l…]?雅
Q£È?ÄfȪÿ?ɑëÖ¹pá?ÄfȪÿ?ì$ NЮÀ?¦j'#'Q7?¾Úý‰zŠ?¦j'#'Q7?ë­^ÝY?{£ýZ:1?ÁJ…ȉúž?{£ýZ:1?Ñïٙ¹Ð?Åwƒ˜"?ç"3#?Åwƒ˜"?Ñ79€\å<?ÎU(Ÿöå?çdc?эb?ÎU(Ÿöå?Ý—Õ°\?»ò;­ff?áwý4'Ò?»ò;­ff?ÓÔÙ¿,-ä?·Zp» é?æ" ié?·Zp» éMIXED4FGL J1951.0+2523?è:ÜÀ"a$¿ä¿Ž‹HÿÀ9á8ˆÝ‰³À;‰á<ÆYì@\fHß@´±'Äjþ?ЅÁ?ÐÐh?èlŠlÕì@ûà\÷R@½çMVŸõ?ïðäÚ	Ì2¿ßöP<Xv¿Ó&íàBËW¿ê»Á¬Þü¿î*GÒ&©¿ïü UŠ÷UNASNone?Õܒ€SU?ËY'¶·b?嶿ÖUs?ËY'¶·b?Ç"Î?ÃqgRìÙ?ê9;·øM?ÃqgRìÙ?à¢Ù‡¬mm?´1*?O¾]?ÞºLð§%&?´1*?O¾]?ÐðÛõ´¢Š?ª4?tJ"Ò?燒%®»?ª4?tJ"Ò?ž˜Ã©å "?£Í"íq±>?ï9âyÝ<?£Í"íq±>?'^0†t ?£âVq,ò?ïm{˜ÒŸ?£âVq,ò?·JKe?¢¨§	Z?íV»ß¥Ô?¢¨§	Z?"ÎÆÐs`?]fãc&?ïa‰ÉS+Ý?]fãc&	MIXED4FGL J1951.3-8015c?í2ˆZÀ=;0aǛ5À:P,á	š³À;þí¢/jQ@p*^£N@(ô€oüè?Îå?	U>?ÉsN@Õ³%?ùи´çÓ¹@Ù1΄1þ¿è"Xº¬8Ù¿ÞNvZ¥=¿äÂAƒ-¿çÜzŸƒh€¿ïü»ýǖ'¿îì:ñm–UNASNone?ïâPÎR*?uøHGΛ?m¯÷#ïe¬?uøHGΛ?ïê"턗?pWА?˜?eÝwI`8?pWА?˜?ïŒðûos?ƒ1ÿ©[j?ŒÃÁ$;ãJ?ƒ1ÿ©[j?ï×TYbó?Z"¼Øëk'?tUôpÛ*x?Z"¼Øëk'?ï«ùæéâ?'W¢Å¼‰?…†SEì+?'W¢Å¼‰?ï²YòШ?ˆeÌGÈX?ƒiƒ|KÕì?ˆeÌGÈX?ë‡kòÊëÕ?®Yq-¼<6?ÁâP4ÔP­?®Yq-¼<6?úÆó?" ZC?¤f`Qçb×?" ZC AGN4FGL J1951.6+2621?ï{Ã*?L¿ÑTËß<'À9=kŠ'•™À:ÉV¸syt@‹ž[JS‹@ÓQùÇכ?ÅÔ\c-L?ÑÀª?.>,@U-úNw@#^邏?ê_åBåWÞ?ï–Ï)ž_¿âcž\vù¿ëN
>¬ãù¿çüÎR
¿ç`oâ*ðUNASNone?ëêÖúiW?ÀgÑBe´?ÀT§ÜZ¤?ÀgÑBe´?ѪdZƒÀ?É,›XOf?ç*ðMÒ¾ ?É,›XOf?è•UÇT4W?´^?áDé?ͪ¨â¯.¤?´^?áDé?ßþ앦+?²Ù~¬{ã?àð	µ,ê?²Ù~¬{ã?Ò©µ¨e[Ç?Éҁ™¿ü|?æ«%+ÍR?Éҁ™¿ü|?Ÿ
±æ¹ÕF?­Ç}ýbÀ	?ï'p…y&?­Ç}ýbÀ	?ÝÛÊ•Ø?·°Š6G?ápšòµ?·°Š6G?§ÑÚªeV·?—'è›B7É?î'âUu't?—'è›B7ÉMIXED4FGL J1953.5+3841?ƒ룝˜ž@¾Ès«ÉÀ9"w3"«À;Á15,2@¾á˜5ìK@žŠdrp`?¿ÈYök®?ĽßwŸI?þEÀi;'@;1KýYˆ¿íª¬çT7?ïô"&"À¿æ¬Žhãï(¿ã¢»a—è¿ëVœ_˜¿Ö1q<-WÒUNASNone3FGL J1953.3+3847?ïÄe¼M?""±
?D?}ôM$
S?""±
?D?ïKK>(?'•Êð
J•?ˆ­-"·ŠÒ?'•Êð
J•?ï2=&Ñûá?äž,¨Í?™¸[$µì?äž,¨Í?ïTFÔ$Û?FíÂi0@?œuw.j™?FíÂi0@?êXÔNe,™?ÁôN¤†e?Ɯ®ÆkM›?ÁôN¤†e?í5«f(?¾üAsV¨?·÷ŽQÈç¾?¾üAsV¨?è¸aýÒ	?¸¥pp.U?Íx	À·Ú?¸¥pp.U?êkU׀?²Ï«7?ÆR¨¡ýÉÍ?²Ï«7AGN4FGL J1954.4-3729¿îQœÞP6À;û¨`ܹªÀ:Æ(¯K²†À<=b†ž@åXvc´…@áhšô­?ÒùYÞÍÒ?Ð
Èâ¬?õð ŽëÁ@±:ªËÆ¿ì Ð?Hl?»Ã!¨FZ­¿âMUô([i¿äy^½zŸ¿ïëÆ!·à¬¿ï"ÝíÜgUNASNone?ïÛgN·ï?¯´€~Ð?rLXìÕÔ§?¯´€~Ð?ïÓ­L\'•?€Å¾äuk­?v)YÆ	S?€Å¾äuk­?îÆDƒÃ?•ñx&"¹?£ŸË´_GØ?•ñx&"¹?ïÐ7–Læ–?_Q2û'v|?wä4êºÀÓ?_Q2û'v|?諸°ˆú?Ž˜I×N?…×TÜ1c?Ž˜I×N?îÅs'}?¯,-ŒS€ž?£¨ÆïNh)?¯,-ŒS€ž?íFí¢Ó?¢¿ya'á?µÏñÜê?¢¿ya'á?ï&B'lpä?™Ó¨?›7­Ô)±?™Ó¨AGN4FGL J1954.5+2420?×:JT3¿ýäH•:À:0S5À;¥Ã<*Rº@Ð3öýwå@L¢À‰Èk?ÓZe¼Tº?äòSÍÝn@à:2*õw@÷l¿›áÈ?ïþ
¡ÿϿ㠝™ÙZ¿ÖÈhûí¿è­µ°P•¿ï÷!ŸŒø¡¿ïë	εÛUNASNone?íMªy!U?½n¤a¯Ú?µ'¬5­ªÖ?½n¤a¯Ú?çÿE^ȧ?Ǖþ¾{?*?ÑÜuBn²?Ǖþ¾{?*?éu•áÝ?¯YŒ¯Ã€?Ë«¦)¨x?¯YŒ¯Ã€?éÍÓêèŽ?£ÍŸPTæ"?ÈȳðT]È?£ÍŸPTæ"?⢖(²?ÍúÔ~ê8:?ÛºÓ®›è?ÍúÔ~ê8:?ÊEüj'Æ?Ézd?o¬‹?én€å~ێ?Ézd?o¬‹?Ù>#+©&?¹É¾©¸9‡?ã`ðîj+m?¹É¾©¸9‡?ÖኆM®×?µèÂ&ϤM?ä:¼Ù(•?µèÂ&ϤMMIXED4FGL J1954.8+2543c?ïÿÒݏ¿ó4(%¸÷À9Q,?#+~À:Ù­´Ù'@
O$«[
@œãÞaIÇ?˧tù|-M?ÖK^£#†@JO‡&ÐN@Õuèºi?ï袠ÿ>?îFâ< š?¿ê¦WþÊ&¿çl1aKõL¿ïñ½m捿á
qs	âØUNASNone?â±XZ½™\?Ìcö–íX?ڝOJ"ÍI?Ìcö–íX?Ç»±á'ç?ÿò~#¿?ê9Q‡¶?ÿò~#¿?æGNńs?´˜£‡PŽ/?Óqcât÷?´˜£‡PŽ/?×=Ü8{$?±Ðs¥)˜?äaùãÂn?±Ðs¥)˜?ÖË`Tî3?ÏV¾ü];Î?äþšOՈç?ÏV¾ü];Î?'ñ®fVâj?¢óva‰œq?ïhrŒ±Ì
?¢óva‰œq?Σ–ªsS?³»"øc-Á?èWUc+@?³»"øc-Á?"fï¤óQâ?…|ç#"—?ï\Ȃæ#á?…|ç#"—1MIXED4FGL J1955.3-5032¿ê&&Ý[ݙÀ>'àãF·À:ÀöÞN«À<r¦Q8ø@bü}"€U@ø½=ã^?¹÷(€|½¿·vœ¿há?þ{ÓJ•Oˆ@>•=im¿ãëÙ7>Z¯¿ä[ÇqC9;¿è"ÏöLø׿䦰~ L¿á¬ïícEJ¿ÊNC"å¢UNASNone?ïÿäƒD:?¯ºe¬?£iچ,œ?¯ºe¬?ïò™ö
Þ«?aS"ÃÉEg?ZÌfQª*?aS"ÃÉEg?ïçâ?t#šËÅ?háÞmù?t#šËÅ?ïý·Úç¢?Þ¤™™'˜?2A*╭š?Þ¤™™'˜?ïþ¹R‹Vú?#îÜ^"LN?$jÖ&5?#îÜ^"LN?ïÄÄV`Š?Ž^÷³à£?}üHq#%?Ž^÷³à£?ïÔ¿½o·ž?~ÎÿŒÿ‹ž?u !;ř?~ÎÿŒÿ‹ž?ïàšçé^?eäªu2?oeëòúÚa?eäªu2AGN4FGL J1955.8-1657?æÀ-ÛþÀ5¨ßXÀ‹vÀ:i1òÁSÀ;õͧ¾‹@+ÌAaŸ,@\…×Dö?Åy£¯ò÷?OÁ—ËŸak?û€©E5?Û&¸{‡	õ?×wEÜ®S¿éDÔ`?ù¿éhšô¬·¿çÉc‹À"?ᐣñâ0UNASNone?ïÕ2!˜ß"?©ñô°ˆÌ×?ufï6ÿÒ{?©ñô°ˆÌ×?ïɝ(«	?…?vƒ,)[?{1k¶ž|?…?vƒ,)[?ïtÍv¸:'?‹`}ª`øO?'fQ. Û?‹`}ª`øO?ïÀ:Zná_?dÉ·9TÄÚ?âÒ±1ø‹?dÉ·9TÄÚ?ïúïܯ?¤?äAiŸ?€¢7˜?¤?äAiŸ?î=QÖG±?´ó
u»A?¬*⚩	?´ó
u»A?îIYÔmç?¡M©ÔjÉú?«jb¹!Ž	?¡M©ÔjÉú?íÑJ™g€Ô?ŸDŒF5I?±u«6
Óß?ŸDŒF5IAGN4FGL J1955.8+1154?ææIˆ_4™À ôuĨ;À;Ž"ÝÀ=óí£*@ "µ$¨?þNÚ"ö¥
?ÛFqÏsÆ?ïn>Â2"þ@߃ê?þ÷öüK@?ÒÖÊ|tW¿ïÿëJw?ïýš)âQ™?Á» <‹v–¿ìÞzt¿ïýSG¥°ÿUNASNone?îxy#?§atÇÏ£F?¨xn°õœH?§atÇÏ£F?çÝ£DúA?Ïqý?ÑòD¹v~?Ïqý?í6ÈKˆ¿'?¢9ƒÉ›"?¶I½¢p)t?¢9ƒÉ›"?ᰇ£31—?¼\|Ã$?ܞ𹙜Ò?¼\|Ã$?êtýNäƒg?Âևb»ë?Æ,
Ämòf?Âևb»ë?Ù­+¶€õ?ÓC;Ûð£Ž?ãy©j$¿†?ÓC;Ûð£Ž?ê¤ùMx¶?°¿¡x»¹?Ålʍ(?°¿¡x»¹?ÐÈBúP"–?ÄB¾V"?ç›Þ'׶5?ÄB¾V"MIXED4FGL J1956.6-7011?¯¦ýo×Ô=À>ç¶þ.n¨À;™÷
ø|À=V%Ýà‡@((ú@@«~žk?ÔÄ_`7Î#?ïÿäâBTä@ÜR¾éµ;@("nmØ?ÓڞF§"¿äëgø6Ýã?âËà=ÂÙ¿àhK_·K¿ïÿd†'V?áécÜHkUNASNone?çïçØے§?É¥#Æ-ÌA?Ð 0NHÚ²?É¥#Æ-ÌA?í·7?:=?¶Ãؗ½=¼?²FFx?¶Ãؗ½=¼?çîÃð/R~?±=«(A¥'?Ð"x¡[?±=«(A¥'?éLš½ŸÍ?²r^T9·3?ÊÏå•	€Ì?²r^T9·3?ãÎÃÇëf–?ÑáŒè0Uˆ?Øbxp)2Ô?ÑáŒè0Uˆ?ã@Âc	I?Ò7Äðèél?Ù~{9Ëín?Ò7Äðèél?×Åræ°?¼ÌJÜG>-?ätƌ¨?¼ÌJÜG>-?Õh³.Î?Á]OJ"ÍI?åK¦}hò™?Á]OJ"ÍIMIXED4FGL J1957.6+1230?ª§£ÂnM[À!_€™"À:ˆ·m¿öûÀ< d©ÍÄD@d'8Ôþ?ÿ'ØÚø	?Ѽ
éÿ
?ÓÄcœ²}Á@ÕÖ¾¾Q@».\^Ñ¿ïß#FV%§?ë[–©û¿ÓN­âü¹ú¿ã¥*&D7g¿âþP§ET¿ïÿýawUNASNone?ïÕãl ˜?t.B!|k?uJ
ôÄ?t.B!|k?ïEu1IÜ?§¦*2ÄÓx?—QYØÇ(‰?§¦*2ÄÓx?î÷¦:op.?''lªÝ–? …œ[œ²?''lªÝ–?ïfQp?sFuþ‡v?"5Ý^IÊ??sFuþ‡v?ï)×3ú÷?™ŽøŽ™ Ó?šÅ™!?™ŽøŽ™ Ó?ëÈ	ëcU?Ä :°ÞG?ÀßÛ¬Rr­?Ä :°ÞG?ìéÆè²0"?¨Ã_ð»?¸±Èºn{^?¨Ã_ð»?íJ*Å?¡JñXÜàÍ?·§M­bZ?¡JñXÜàÍAGN4FGL J1959.3-6121¿éà[®bºœÀ?¦bfýeÀ;¢™=SHÀ<êI"Çȁ@!VH‹´ÿ|?ò+ŽXó·?ã8b1?í'ѹ›—¡@N»Ÿ}ß)@\ƒÐ`«¿ïÿÓõµú"?ï÷AJM+,¿È=a	…:?æ"Ñá^ª/¿âQ'W«¸€¿áÃÙDr UNASNone?ïúÉלV?SQ–_¥D"?DØ¢)#,b?SQ–_¥D"?ïñ}9;¶?b2
CnÍe?]ǶÃãÿ?b2
CnÍe?ïi¥¹É¡?Ž»:ø`?'ËHÃ\Ct?Ž»:ø`?ïîÙ.&{a?QÙ÷|ª?a&Ò~^r?QÙ÷|ª?ïø¬)I´?Põ§0¸Þô?MOZÄAË?Põ§0¸Þô?ïÎ%–c.?öݺUá?xí@%° î?öݺUá?ïˆßÛzî?ŽB>»2¹?È	†÷?ŽB>»2¹?ïÚÍné\?qoº mv?r™}Î
²/?qoº mvAGN4FGL J1959.9-4605?µ¡öûÇÀ>­ú‡;À;ßúTÅT3À<푮éŒ÷@"Y:-ù8?óxÏÞ±Ò?à´/è%ç?Ù¯Üüð¬?÷Ì_‰ÓRù@}%
«:¿îØúØxÒ?ﳬ ›%¿íç^~:˜'?ÉWw¬	?½ y1Å¿áŸê¶ÂŸLUNASNone?ïýÚ@¨¼¢?0Qý!ªÜ¬?1-ù'ñƒQ?0Qý!ªÜ¬?ïôty#­Y?\…}Þ|?W
Ëãg?\…}Þ|?ïžÔßôO{?ƒÞ['vš?ˆJÇüé8?ƒÞ['vš?ïÿ5¨"?8Æ,íÏ?JÿÜ>?å?8Æ,íÏ?ïý…]¼7˜?<åôýæ:?3Õ8vú|?<åôýæ:?ïÏõç
k?ŽÂF¤H,?xv¨¦s?ŽÂF¤H,?ï¦1|,?†*/=*9?†x3®³P2?†*/=*9?ïü˜¸¯D¸?=Ôk'Æf?;:;1`Z"?=Ôk'ÆfAGN4FGL J1959.9+1833?çû›[)‹À¼Pbîâ¡À:|³_=}9À;ç¶jŠ¸U@æ"Ôei@™íeÊ?ÏMò?Ò³×Ùõ@Ëi¥¶Ž?û•P9(j­?ïýà€ˆÑu¿æG¡Ÿw¿á·T*#¿ù¿àÑNÂò®¿ïýZØ®¿ïýl<i<ÚUNASNone?îª@Û½V?²d±éHP?®•[ðŒ\ª?²d±éHP?éû0RX<'?Ãl2ioì?È>¶Ÿ
ø?Ãl2ioì?í8äâ\ö?¡MN$k¾A?¶8Øí#Ï?¡MN$k¾A?ëZ^T©"?žûtU?–‡š­Y¯?žûtU?è×Tʧj?Äi¦aÔ{?Ì¢¯ˆÕbY?Äi¦aÔ{?Ò7Εq8I?͸'æ`¶h?æäµGcÜ?͸'æ`¶h?åàpB³-ê?¸Þ¿´"–?Ô?z™¤+?¸Þ¿´"–?ØO]hï`?³Þý|Z(?ãüØQKˆP?³Þý|Z(MIXED4FGL J2001.5+1611?ÝôÍO‡/gÀñ¾±ìÀ:ÞkZÁíÀ;Շºtµ@ý-Ûö@Æw}åÞí?ÐR—\R'G?ÛS%âØp@(Ëwb?ùqoXþHñ?ãwÁm9Í¿ààM³9ä¿é	(Ó]à†¿ènn¨TG€¿è±òá‰rZ¿ïÿô╋îUNASNone?î ËÅê?µå);Tî.?¥óC±•Î?µå);Tî.?å©z™	?ËÔ¹àáס?Ô­
Íìåú?ËÔ¹àáס?í+ð¡hE?¡&k"?¶ zôOä?¡&k"?év"êk?¦ª€ûƈ?Ê'ŸtWžU?¦ª€ûƈ?æü)N?Í­|Ð`*?ÓÚ¬ácÌ?Í­|Ð`*?½ƒÇdø?Ã?•õ¨Á³?ìO‡|€ü?Ã?•õ¨Á³?ãvl)/?¹:֐|Û?Ùãç'­¢?¹:֐|Û?Ȋ³*lîž?«<'¾z?éÝS5dÄX?«<'¾zMIXED4FGL J2001.5-0958?íñ|1ÝP[À4ß«÷jÀ:•GûATÀ<ÝË!Ñâ@QaÒ-ø@â
Üa•F?Ó'½ÝEÁ?ÃU´'Œ¶?òÖ0=µm5?ù(ï7…Ó?ïšúAп睨ÇßÓ¿ëý7Þ¾'Ì¿åÚKäÚá¿ëY*GÒ'?Î}šàkUNASNone?ïӃâÅ~ò?}rì[`3?v>˜qù?}rì[`3?î¦í÷X«W?±ä&JÎw ?¥' äæ'?±ä&JÎw ?î'x…'"?–."›ÝK?£T8u1É?–."›ÝK?îÂzãÃUÍ?…ӝò$èE?£ØQÃÊ£/?…ӝò$èE?íå'ª{?°îRq
Ÿ«?°Ö®±­?°îRq
Ÿ«?ⶾÿmª?Ñş´hI?ڒ'ç$¬?Ñş´hI?ë½ñ"¼Ç?¯
cL%?Á9±ãú?¯
cL%?äg
›)?¶¶Ì¥ø‡?×1äÉíê?¶¶Ì¥ø‡AGN4FGL J2005.8+3357¿Ù«;/ßtM?ñxE܃#6À9VÆÀCQŽÀ:›tkâ§*@ >vx'GÃ@ãÕº²?ÁYɟñ¢o¿¨-;¼2Ž?ð%ôkwG_@ö§uzU‡¿î
9	6	§?ïí֝0'¿çÕ¹€ቿë9ÝaD"ƒ¿èïî:ß?Ŕrþ¥7UNASNone?ïÑIõ.ø?—²a!êÎ?w[}w÷?—²a!êÎ?ïÅæÈ1î?‰O=kJš¼?}›Ó0mI?‰O=kJš¼?ë²,]®?¯œWæ¦$³?Á7Oú‹™H?¯œWæ¦$³?ïÓ^ÍH{M?cèF˜NÑ?vP™VòåÄ?cèF˜NÑ?ï:YZ—Ú?ži2Ú®óÚ?˜¼tØ Å?ži2Ú®óÚ?í¯ì‹rÔ?»n^[Ä» ?²ƒ€Ê*Ü?»n^[Ä» ?욘
8³â?­þpÖ#Z?»+?–:`ñ?­þpÖ#Z?î#YК¦y?£%Øõ­Ÿ>?­Êbø
fr?£%Øõ­Ÿ>AGN4FGL J2006.0-6538¿êôôx"ÃkÀ@ï$©ÁÀ<©1½nÀ=¬tg°é@#'ó‡÷†?÷%ˆ»%œ?â}Ÿ"Ò?Êb¯ã Ü?îÓ·¢™œ?ô qÇîk®¿ïZu%F¿ïö†5•8?ð¿Ó½SG¥°ÿ¿åËJÍǟ?Ðmû½ñhUNASNone?ïûñÙTM=?;}q¤ÃÓY?@8šÀb¦8?;}q¤ÃÓY?ïëуQ?k‹_œ)5=?d.|·+ü?k‹_œ)5=?ï™ùÊ˄'?ˆ¼ºeT9?‰Wm¯n?ˆ¼ºeT9?ïÞ/Í;÷A?dò>Ú±?pèf#çŽ?dò>Ú±?ïýj|©&ˆ?7Ù5ŒRoc?4¬Y†®?7Ù5ŒRoc?ï¾Ð]ê±?‹†ûäÕ"?€î³Ï?‹†ûäÕ"?ï Èyá?Šfº˜C†?‡Íá¶h?Šfº˜C†?ïyT°"?§à«½7Í?ÕiïÖé¼?§à«½7ÍAGN4FGL J2006.4-0354?íb‡×­ÚÀ2v…¹èÄzÀ:àUӌÚÀ<'ÅÅqŽ¹@›,™f
@a
;Ã$­?ÉyD$>û?•P?J£?ÏôÔ¾2Ö@þv·Au@?¤–á?æ°§2È¿é¬"qÌ¿æq²à<–3¿ÄïXgö…¿ïóqal+¢UNASNone?ïùU~.%¥?M¿¸Ùë}?JªIÌ?M¿¸Ùë}?ïÞÛừ`?yCÖ<¹Ï?p'- û?yCÖ<¹Ï?ïÉ°&'ª¬?y¥óg"Ôˆ?{'쯆 ?y¥óg"Ôˆ?ïöÓý ZF??ŸI0Ǜ?RX¬
£Ð??ŸI0Ǜ?ï³du݅?‰W¨Ü£F¦?ƒ&ý%ø:£?‰W¨Ü£F¦?ï,U'±?¤`±!÷?šuM×EÃü?¤`±!÷?ï[NZV
?š"®‰oõ?Ÿ4–8$Úa?š"®‰oõ?ïÍžQ—Ö?qó*µl}?yy°¸÷…A?qó*µl}AGN4FGL J2006.4+1834¿'ñ6!œÀýۘAªÅÀ;'~B%>À<Xæk"@ òc'?ýlÖÂïÔ?Öô¢Ô«¾_?Êö²¤W±?ùŽ"î9.@–Ѿ#<¿à O–@I?ïñQçS`пíî+÷Տ?ã_ïSàR¿äËôï#¿ç×Fm¢šÊUNASNone?ïü9[þ6?Vö‰àG?>7ö*#@J?Vö‰àG?ïÇ»Eeå¸?Ši?½7á÷?|"]cºà?Ši?½7á÷?ﮃÿ‡à?ƒ/eóuÀ8?"_lû?ƒ/eóuÀ8?ïð³$?MÀ&ZŽ°?^™ñ"À‰x?MÀ&ZŽ°?ïéÆ%Fi$?lى3pöÝ?f9Úz^Ê?lى3pöÝ?îŸÎèc‰Æ?²‰SfF•m?¦vWǨ?²‰SfF•m?ï<vvåö¦?"zWä´O?˜q1!‰]N?"zWä´O?ï³ÎŽ˜ßŠ?~z…Öh·?ƒ\XOh?~z…Öh·AGN4FGL J2007.0+0707¿Ü?N ˆ1yÀ*"œ
!¼À:2wKøÀ;ðK+w}@`Õ²yc@YOýnUH?ÉÃ]wÕN§?®¿»ŸÜ\j?å:áqÊ@҉SP_¿å$ô,¿æ6¢ôŒ.w¿äþö€$}Ž¿çiqÛ¯¿àîç©Çå¿ïÿóÖ&ãUNASNone?ïôãÄ3?Pì@½ÚËy?V9ÛqÁës?Pì@½ÚËy?ïӇñÞð?'cbx4¸?v<!ò@?'cbx4¸?ïdzŒ£«°?u+D
H¾Ã?|&9 k¸
?u+D
H¾Ã?ïë4ÞÑS'?K7Ü¢LU?dË!'?K7Ü¢LU?ïÝO°†3û?k0Xš?qX'ӓng?k0Xš?î¨L¹QV?¯Ê_üh;–?¥{>ӏ ?¯Ê_üh;–?ï%RÊI²?—<N¹O?›U¦¯ê"g?—<N¹O?ïCóR{*¡?ˆ gSí?—•²RyÕ?ˆ gSíAGN4FGL J2007.2-3157¿ï:Ô.ëÐÉÀ=1ðÃLÀ:=ƒá¡pÀ<<Ãþ¬C@+,õVƒÅ@¡|å-ì¢?Äaºö¶€?È´ÃÁ‹P+@¨³Ûd?E?ïuo]þ/?îגŽ¿Â4]ë¿ÝôÑc4'¿¿âŸ……`ý¿é¤IöÄ¿ïâòÞ¯M`UNASNone?íàUí¿­ø?²˜ç¥½«?°ýP"LjÀ?²˜ç¥½«?毘¢½?ʲ¹à?Ò¡ûÚκ…?ʲ¹à?í³õk˜Ä?¡¹;å"Gí?²`WÍ-^?¡¹;å"Gí?äYMAã`s?±òZwô?×Me|9??±òZwô?åKÔH…ï‡?Çöù#ËiÔ?ÕhWnô ñ?Çöù#ËiÔ?È]‹š2`?ÊÚuL2] ?éè>Ùsh?ÊÚuL2] ?è¿Ë†'÷?´³ÏbÄ¿?ÍÓ±å¸#?´³ÏbÄ¿?Ç98¬€f?®¦}»i8ƒ?ê1±Ôßüç?®¦}»i8ƒMIXED4FGL J2007.9+2511?ÛÙÁ¹PøÀÌ W"ýÀ:Vã®À;Úà!p"@ŒÛâêE"@Â&ޑo?Ëk›¦ÿ?áqðþZcy@•ÚÈ8?ìÙAéj£s?ïÿs}¦¿Ñ¥!øxLB¿š…}`††¿ä'á4¸Ä¿ë=3g5™?¿ëëԚ ¨UNASNone?å^>£˜È?ËR¦Lý¬
?ÕC'¸Îàp?ËR¦Lý¬
?Ãäq¯Þ?²§où•¶?ë8Fã"9ˆ?²§où•¶?æɛO¯É9?±aϨÊ9?ÒlÉ` m?±aϨÊ9?·4ï=?˜IÙ
úƒ?íb›5??˜IÙ
úƒ?Éwr¢Q?Ìo3û–J?é¢8ã\—l?Ìo3û–J?r^,Õ?­£"~í?ïœmÅ	?­£"~í?ÊÉ%ÎEÈ·?µÛæÅAI>?éM¶ŒnÒ?µÛæÅAI>?sUyšzÞü?aë[+=|(?ïÙUæ‡"?aë[+=|(MIXED4FGL J2008.4+1619?ïÛð3â¹&À!§"š|©À:ÐI!²oÀ<Aٌίü@ {3§ø,?Ñô{<ŒMV?âÛ ö¼Š?ïÝÊì!üª?ûº£º"ˬ@¨[#*¿Ý]pH'¿ì9)í9Sß¿æîá(úJ?µîÓTPd¿áÆsxŠ¿ïÿþøþ"UNASNone?ïí7:(ñ?{F'¾´LÎ?bíÈÒ5§5?{F'¾´LÎ?ïҟ†Æ?‰uTÉc"?v°r/é˜Þ?‰uTÉc"?ï84ŽÊU?' Mד1?˜ùn!ò±?' Mד1?ïöø0 æ?D¯2)þÜ?RŸ'G"ý?D¯2)þÜ?ïë逕DS?n±ÞdoÛ?di[Õ?n±ÞdoÛ?îÍëTf"Ž?²v8¢#z?£!J·æ	*?²v8¢#z?ïŠñ56î?–½T"°ÈÏ?¡Ô1¸7?–½T"°ÈÏ?ïù¿®ý?LÛg-Wo?IG]AÞÅ?LÛg-WoAGN4FGL J2009.5+2425?é1«òjHÒÀïdþ‡YüÀ:Šh¤.HÀ;hFDe@cÉÑÅ°@§ÛðuI?Òò)=;å?ÜA^#÷«ô@äàTi
á?Üϧº'i?ïþr–öQ+¿×æÓs¯û¿ç=¥b$¸F¿ìŽpK™\¿ïÿ']<9¿í·ØIёUNASNone?ìm¾Bõ??ÈeD°ç?¼'eèV?ÈeD°ç?Ã,0f
‡)?Äù'&O8ç?ë4óæ}^6?Äù'&O8ç?êúˆÞÐU?§vÓU"?Ä܄¿†­?§vÓU"?¬A'î!	?"¬m	Wg?î;ãׯ?"¬m	Wg?æèÄJOâõ?ͬçx¹i?Ò.wk`:?ͬçx¹i?žç¿h÷jy?«¿ù÷ªá?ïÂáü?«¿ù÷ªá?Û³‡[Ôg ?·¶L'º"÷?â&<RÌp?·¶L'º"÷?PyMƒ÷\ø?@îýxÓu'?ï÷ÃYl¿?@îýxÓu'	MIXED4FGL J2009.9-2116¿é#
"1œõÀ:ZA€ÓÏöÀ;	±oy4ŸÀ<ÎÛÈRé@àµFsW?ý…Á•a&?ÎMúI\ÀJ?ãÃBàO`@´Õ½6VÔ?üæÒâ¿ï'¡­º8?ïþo§WÈ>?Õ-•d€³¿ãb:[€Y¿êÇ
H½ß¿ïÿ²2ӁUNASNone3FGL J2010.0-2120?ãÅjq§§?ˌ›ÂœOà?ÙÌu+°²?ˌ›ÂœOà?á–Õ¦Tø?Ì}:¦¢Ÿ/?ÜÒT³Wþ?Ì}:¦¢Ÿ/?å[!«:D¹?³HñÈp î?ÕI¼©‹vŽ?³HñÈp î?àü­…uË?±K‹r'!c?Þ¥öõj?±K‹r'!c?ÎqË¡uþV?ݤP*?èc¢€j?ݤP*?Á]7¸?ĸ`øÔ?ë¸(²?œ'?ĸ`øÔ?Î>Í'2s?µŒjQW‹'?èpL¶3z£?µŒjQW‹'?•'æ?¯àÉ.Î{?ëZ›~:{?¯àÉ.Î{MIXED4FGL J2012.1-5234?í£Þjð À@£}é9êÝÀ;CšMô€À<¢È£r`p@"¨YßDs¢?üé
	Ó¾Y?¸éú=|b¿ÀJNØ«'a@ñÿ ÜïZ?òà-"ã§Z¿êiU./¾4¿ãºßr#¿ìyÄaÄ@6?ÞpØûYR,¿é,Žž"Ô^?Ð;e[Ï_UNASNone?ïõ°6,¸?ƒ}'Qn†?TŸÏŽ'0€?ƒ}'Qn†?r w?œëžˆ¼ˆ¤?Œ—#{7âM?œëžˆ¼ˆ¤?ïr}tä=?ùâ:ºi‡?'°QZÕRq?ùâ:ºi‡?ïÔüél?l;%dMen?u‹9ëB^?l;%dMen?ïépƒ9Ÿ£?nñkγà?f|êM?nñkγà?ía¬·æ?ÃÝ·‡&‹–?·ò›'@Ñ?ÃÝ·‡&‹–?ïETg$@@?'z>ÿRÁ?—Us/Åþ?'z>ÿRÁ?íV¹œÕt?°‡tîx?µOz1ÏyÞ?°‡tîxAGN4FGL J2013.9-8717¿ÞS6'}	…À<°_®¼À;¤'[rÏÀ<֑¹ÑG†@!29OWB?÷4Œê^®?Ù=œ˜§?Ø}jŽê/?þw'Þ"um?úàï""n¿ïýxÑ¢õc¿ÝñïÜqZ‹?ì÷ª%Øם?²<£Ip·M¿×6‹{U6¿èŽá¯²áUNASNone?ïûÝ9½¢?5i¡þCǓ?@‹˜ô:?5i¡þCǓ?ïð´†É¢?c]t飪?_֗
雼?c]t飪?ïº5 Ë½?zé÷M||'?r—ÔŸã`?zé÷M||'?ïêÊPñŠ?Rh	¥Úhk?e5®ÍÝ<â?Rh	¥Úhk?ïú£ªóâ?BFþ'-•?EqT¸Æñ€?BFþ'-•?ïÆʜÆʪ?†M)¸çæÏ?|š±›ê¾è?†M)¸çæÏ?ïÙ%êºp?wüuŒ*L?sm
ƒ]`b?wüuŒ*L?ï¨ée+J?uØä¡?P?~«‹<ì:í?uØä¡?PAGN4FGL J2014.9+1225¿ë»rkúœ`À(n$ÛÀ:¬%¦'¶(À<rÛ¿®×@'}‹qÞ@|Zœ-Ȑ?É¥>}êª?¨ÙMþTs?àá¡Au@Uzæ{¯¿îxx¢(3{?³/ÈðtFÏ¿ë[iw'ß¿Ï*ö´Ò°¿ãê–vÏj6¿ðUNASNone?ïöB'¨÷—?VO|³Å?S{°ÆÎq?VO|³Å?ïÖÁ¬ˆs?'__I?tŸ)Þn2?'__I?ﻉŒ
óf?zæ	¼ó¸?œúsbq?zæ	¼ó¸?ïó.® ?@²'J	M?YâK\?@²'J	M?ï¡ÎýA?ŽÍGdÃ?‡¿Œp±Ûê?ŽÍGdÃ?îڋ"¿Ñ?­D­¤«ý?¢WMÞtö?­D­¤«ý?îÙÙÌÔH[?ž4s‰–j†?¢bc/KÞU?ž4s‰–j†?ï›Ït¥vû?{X³êå{ï?‰"ÚÝ7?{X³êå{ïAGN4FGL J2015.3+0758?ïmœQÀ-:}ªOÊCÀ:hꭈcçÀ;ÙRé±ßá@…xÐK\u@üô}þ•?¿å[9ºH¿²Ûae¿c?ów¨Èá…Á?ü³…ü-ãh?éà"¾ŽE©¿êûêâa‰ˆ¿å2d×.¿ê÷Ü_ïT¿ïò³±rÔ3?ïҌ)nŽSUNASNone?ïäòt•í×?qm0jV?k
‹žL8j?qm0jV?ïP¶#À?¤®åã4?•ýi@Äÿ?¤®åã4?ï8¨:€?r,*EòÕ?˜êì]æÙ÷?r,*EòÕ?ï—R™Ú?sƒ¸ÿ^ô?Š+YLJî•?sƒ¸ÿ^ô?ïl ^§?™ãEÙ)Ü°?}2kô+?™ãEÙ)Ü°?ç¡l¡=þ?΀çfV H?н÷&½"?΀çfV H?îÒùa«A? |Hw«?®Ðlyñ? |Hw«?êS>J5?³*ËòN"ø?ƱËד-?³*ËòN"øAGN4FGL J2017.3+3525¿Ê&ÈÅðÔX¿´u"–ØÊÀ:Ç>A".ÎÀ<)I`œ"@!½Hö>
?ò_æ¤ì´?Øu\"•¬?ïÿïÚê@
É?äò]€?ü(^Η}5¿ëÖ?rÖÚ¿ì| ·Ûy¿Ò]
øGv?Ëz£_@,k¿åê{3}¿ïÿ~?ËòÝUNASNone?ëԍáÞ	"?ÁtlÈoæ?À­Èx‡Ù±?ÁtlÈoæ?è8N°½!´?ÍYÞÿ»rÃ?ÏÅ=y0?ÍYÞÿ»rÃ?ì«.\^Ñ?¦#õ§²B$?º§¦	{?¦#õ§²B$?ë§rÝd–û?¨Ÿ*ég×
?Áb4Šm¤?¨Ÿ*ég×
?ê÷%¾?Ãy¡6_Ò?Äñ#óiš?Ãy¡6_Ò?ØA²ÈÕu?Ôþ¼€pË?ãß&›öF?Ôþ¼€pË?êÅ¿JêE??°NX ?ÄéÔVë?°NX ?ã.Ÿd"®?Ãzw¯'å?Ù¢Á7º£Í?Ãzw¯'åMIXED4FGL J2017.9-0114¿Ø#8¡(¦ŠÀ3¼î9.÷À;öÜjςÀ<[ƒ°úo@ræ@fU@
%ó¯?ÓsŽ!ì8ù?àèS¦pA±@ÚcÞÌ©'@§æž!ê¿ë>L×I''?î‡óÿÁ–¹¿×ó{B¤,¿èš† @¿ïüð§12¿ðUNASNone?ïg"}•?£‹µ3Än?œÝ'q?£‹µ3Än?êM€Ü‰XY?"LÅÍÌt?ÆÉüÚž?"LÅÍÌt?ìðAc¢'»? ñ|Ð"Q@?¸}ôä£@'? ñ|Ð"Q@?ë+ïÆ]->?¢02t\ÎV?ÃP@æ‹K?¢02t\ÎV?êuo4ZŒ?¿à¢dìT?Æ*C.—±Ò?¿à¢dìT?×uzÏî¯?Ò[¶â!?7?äEB˜¨y?Ò[¶â!?7?ç6…3lO?¶èüS{'?Ñá'õ™'a?¶èüS{'?ӟí¸&¼?¹¥ã%•?æ0	s#ì¢?¹¥ã%•MIXED4FGL J2018.0+7903?׏ݠ&@6©˜áõ²À;É+ml%À=Kh;R¼e@þµFÉ= @lñ<îØ?Õ×Ä3êé?ï&p­F@P¨>x
Ô@p£V0ä?Ô_2€ó¿×dŸg™¿¯Ó.±Í¿èélÀ"{¿ïÿàöO}¿ïþ€Ǒ$UNASNone?î–^ãT"?°n\ïü?¦šÉâÿÃ?°n\ïü?ê9"}(}?ÃSCçÞ?Çë²^?ÃSCçÞ?ìº5¤Ï?¢ÇÒgñtÛ?º.Rۑƒ?¢ÇÒgñtÛ?ãui—&?²Ï¾9y,î?ÙÑÃ,Ñ´?²Ï¾9y,î?æä@^"àÍ?Ëðš´n(Ÿ?Ò7BÖ>f?Ëðš´n(Ÿ?ׯ´'])?Îlä¸Y?ä(%¶Ñkv?Îlä¸Y?å$'ÖoÊ?»'ó
µL?Õ·æúS l?»'ó
µL?Åϗ"æ*?­É— 3i?êŒ܆v?­É— 3iMIXED4FGL J2019.6+0616?ÙݎbÑ'óÀ0cÛ]‰HÀ:žcʪ³À;Ûxâií@ã`"jZ½@8ââ¸Ç\?η:ë
€?¿@1ôCß?óµý˜F³C@Ún9™~¿^£úF?ïõŸI[ê¿æ"@ ×f¿ê}ó¶E¡Ë¿æª§=Ç
ì¿Ê£]½ _UNASNone?ïùß
'l?QñoZŠï?HƒËBlöX?QñoZŠï?ﮞ™³›?Œúp¼.-¶?"}KÔ©`?Œúp¼.-¶?ïªÃ"ñä+?'/…½I?…OÀYN?'/…½I?ﺱ‰F݁?g´ÿZ¤up?S»W#'?g´ÿZ¤up?ïœå—°¢?Žq§—·?ˆÆš‰{n?Žq§—·?ìÂP¶ÀŠ¹?Á±Þ§ô-í?¹ízIûª9?Á±Þ§ô-í?íÀîжCý?§
ÕÖt?±ø‰z»Ó˜?§
ÕÖt?í÷ó[?§XVÔß&'?·_^£«?§XVÔß&'AGN4FGL J2021.9+3609?éʎaµ°¿Û5L½j¯À;hÙÞ-GÀ<
Ž7eÇÛ@$‰ç˜ã?éà§_ªài?âÛþCx?ïÿH è@uúX S?üJÓlN2¿ïûš?±Æ·?îJùÞ}Ï9¿ÕÒ½<64¿ïú²]à°Ú?ïåe¶™…?Âw´ÂiòbUNASNone?ï¸1QS&:?šxçÜîd?ó«¦€?šxçÜîd?î&€ŽÊww?¾ˆÊᲄo?­—÷Äӗ?¾ˆÊᲄo?ìæ^Nz'?¥ðZ›ü?¸Í
‹+í?¥ðZ›ü?ï½bøƒð÷?€‡FØŸg?€§AÚ4ND?€‡FØŸg?ïKæAÄU?¢ÆÈ}È?–ƒ7Ó7h?¢ÆÈ}È?栻ļ²ù?Ó/ˆgÜÌä?Ò¾ˆv†š?Ó/ˆgÜÌä?ë(1PɵÛ?«
	´ÑÝ?Ã_:¼Ù(•?«
	´ÑÝ?íÓÙªg?·dDWQ?±a2ª¢*?·dDWQAGN4FGL J2023.3-1947?áè€X;;§À<ÅAÈ!laÀ:Gû'½À<:»9&';@YžP7¥ß@óõÞ>Y?ÅI©Äå?Ä1s*.$?ûL¹ìö8?üþS¶‹¿ÜÅ3ü0耿åóû_‡O¿æ"f"?=¿ç>¸Ø#B$¿ïÿ*LÚ¤&¿êá'V¯UNASNone?ï§ö:p?šgRüO'ü?†ÍoÓÛ?šgRüO'ü?ï0〲?¤"àÞbÞ?™üýeG·¸?¤"àÞbÞ?ï'"Q<D?"!DÛ'?ž-­'hۈ?"!DÛ'?î°ÞNvÒè?ŠšúòÃå?¤òJŸ…?ŠšúòÃå?íè-ãà\?¬þÌ¿Jp?°¿Îs	 ?¬þÌ¿Jp?én¢ë&ÿô?ÈÃÖRÎ?ÊEtSd0?ÈÃÖRÎ?ìÓÃ=×a?©´â	õÍ!?¹aæßj}?©´â	õÍ!?æ?rEºÝ?·RÇ÷E´?Ӂt‹ÔE?·RÇ÷E´AGN4FGL J2024.2+3616?î¦Ánä~¿ç¿û}º@À9¼L¼ƒ©À:ÊèïBB›@ ¸dÁÅ@XÕ[ç‡c?Ð5†?º•òpw¿?ï¨E™gD³@
,€ÛÞ¿ïù}Ðwl?ïþR€ÖT5¿âß̃ѱ8¿ãV¶Zš€I¿éÆyÌt¸9¿àEa3 ¿UNASNone?ïX|'ÔÓy?§ð²~C²?"ðo¥eå?§ð²~C²?k•a?™L¼—ªM?Žþ;oç?™L¼—ªM?ìÔ/£lèG?©•moW`?¹^'ãNãK?©•moW`?ïU©@ðN÷?±y›]¥3?•J×èÕY?±y›]¥3?ì\@rXY?¼­(['¡?½¥üm=4?¼­(['¡?쮌-Üme?÷[ºæÆ?º‹ž'"Ù?÷[ºæÆ?ê0é2ø¿‰?³M·LجÇ?Ç<[4Ý?³M·LجÇ?é¾c£œŒ?¹ee×d?ÉqqíÒ?¹ee×dAGN4FGL J2026.0+4718¿ì8H^¯Û@^ÂRˆÀ:Ót«£‡YÀ<n´Ý¾V@ø²m¥õÈ?ÿ-5Ã0kÙ?Ӄ_èÈ×?æZË]a'@WgZ',–@²³HÂ;¤¿ïÿÒH6Ðw?ïìrº1¿–¿¥äká
؇¿ÒHSUèiá¿î1"áHÚº¿ïÕFƒrèUNASNone3FGL J2026.4+4709?í×3ä;±å?´Œ&î-$
?±F`Ûü¯W?´Œ&î-$
?èG!/á«<?Étˊhµ\?Îã{@yS?Étˊhµ\?ìÞ+@Âà1?£
ã4BR?¹¥ù{
ö?£
ã4BR?è*_
›bá?§|VQk8¥?ÏVƒÉ't{?§|VQk8¥?êÊK¨;?ÁHWä?ÄמÓÑ_?ÁHWä?Ø—w€j?Ò[°æùZ?ã÷´D?Êñ?Ò[°æùZ?椕 8.Æ?·ç2Ïl+¦?Ò¶Õ¿¢u?·ç2Ïl+¦?ÖLÀDu2?»U™úèi?äٟÝÅ1g?»U™úèiMIXED4FGL J2026.3+1431?çö|'fŽÀ*ãjËGÀ:ËSïk]FÀ<«[ï@ôÙ4ª,?ú•çéóN?Ïȅ?o'?â=>»&²@‰`ÈW?þ§^3$k¿ï쾤ëÝ3?ï{ÆKç_¿·¾t¶¿×»o! ä'¿ëko"óh¿ïþÉA‰UNASNone3FGL J2026.3+1430?âyNÙ_ŠÞ?ÎçÖ;iK?Û
bM@êE?ÎçÖ;iK?à99Œ¤Ð?ÍJ{NT÷©?ߌýŒæ¶a?ÍJ{NT÷©?ã,2nÎP?´­h]=q?Ù§›"c_Ô?´­h]=q?å'k¸	ò?¬©äáÞ°9?ÔÛ(ìÈ?¬©äáÞ°9?ËLï'Õ©?Å`X'4ÂÍ?é,Ä8v
–?Å`X'4ÂÍ?»ÃeV,Bº?‰ïY¶÷ñ?쇓U:w©?‰ïY¶÷ñ?Ð3Òð¨I5?¶[·Íˆq?ç懫Ûf?¶[·Íˆq?Ï–cs?·PŒÜò?è?zg#??·PŒÜòMIXED4FGL J2027.0+2811?ÈÏ<>À‡oó­â&À9¬ŠS«x¿À<©"àß@Ans{!ß@z*ž9;‹?Á *†<ð?ë7ZU¶ì@!ýAØèd@YøŠ•Æ?ïû/²?¶Âa C?¿Ü7e\{+¿íô×x!yÍ¿ï÷M@ÝÁ¿ïÎ߁Z]šUNASNone3FGL J2026.8+2813?«aÆrÚVè?¹#ë<…‰›?îI㘍¢b?¹#ë<…‰›?¯‡¡_æ¹k?²Al¢cÄ?î…éʚª?²Al¢cÄ?È;Ÿpü ?®¸`h§\›?éñ#ÀØ?®¸`h§\›?¡É6Ø=Ë?‰–/ôè´?îãl'`¦o?‰–/ôè´?|Œ­å0?À\ÉØYP‡?ïš²•¶?À\ÉØYP‡?ˆç²9FÇ?–ªŽ»B?ïœa7R|¥?–ªŽ»B?¼Y±)á®?­œFgÛk?ì|ôÉÚÃÊ?­œFgÛk?Mìã³.fv?>ûb‹8S?ïø"Ç-.??>ûb‹8SPSR4FGL J2029.1-3050?îìÜ`yÏÀ@­
A1"¸À:¬\qðÞ$À<6.#)@"Pðˆi@P9Ô7$?Ñ9¾½•wK?ÊûW2'?õ¬8Ï
@öåS+v%¿¸K"@'ý¿æâCÏb©¿éÍÕáH"Ô¿ätáÙú2¿ïÿŠ#ÚМ?¦¡€Ã´ËUNASNone?ïÖAVÑ6Ù?sA7몸?tßT¬²'"?sA7몸?ïÙu攨?†$ì"H?suE–$6?†$ì"H?ïxÂ;¤Eð?…ìñX½ôQ?ç¸ŽæÝü?…ìñX½ôQ?ïâ}JzïØ?U?"@G™v?m'µ³ÊØ	?U?"@G™v?ïÓ)'Z2?dùZžÛ?vk7hBzÌ?dùZžÛ?îù¶Iþ{Æ?¥6Ä,'@Û? d›c‡ß"?¥6Ä,'@Û?í谈üñá?¢eðá?°º{º>2s?¢eðá?îâôÂñ=?Æ¨¶ç	?¡Ð³Ì ­	?Æ¨¶ç	AGN4FGL J2029.4+1013¿ë9ãóÒBÀ0dô¥Xê}À:Œ^×ü«¸À;ï&<ª«:@÷\1X$@Ìa¢—o?Ý$‡¾û¨Ø?ÛjŸ(Ï­?òÓ<7¾³/?ø"ãäës·ˆ¿ê"k'Qտᡚÿöø¿èLewS¿ïúý—oó®?ï€Ú…óUNASNone3FGL J2028.7+1012?ïºd|?±\®7ӄa?Ÿ(³xI.?±\®7ӄa?ïq¯%$°A?œX ½ë¬Ž?'Ê÷Ú?œX ½ë¬Ž?í¤åìÈ?¢AÄj"z?·ß"×ô²À?¢AÄj"z?ï}4<XÜ÷?{í"õCY3?YxlM[(?{í"õCY3?¥S?±¢…PŒ_t?®Õع_Ë?±¢…PŒ_t?é'YtýO?ÊVü\'?Éö›Š,
Â?ÊVü\'?è°Ø	8Z\?³^w¢}ƒ?Í<ŸÛ–?³^w¢}ƒ?ë¼	w[T?±šY¨f?ÁÚ#ޒ®?±šY¨fAGN4FGL J2029.5-4237?ïÞºæ,ÀA¾#ˆÀ:͗ZBÀ=Ð&¡@Ö	³2@®ü*ˆj?ɼÿdύq?ïÿça"¯­@ìYÙ?üŒUc_?ïâTžgߍ?ÏkY?aj¿á矶êy¿ïý6AZ"I¿éނ¬Ã¿íœݰʹUNASNone3FGL J2029.5-4232?ÕiT	?Ô€
4#§?åKUûxö{?Ô€
4#§?Ә §Y9œ?ɔyòèÈß?æ3ï¬Sc2?ɔyòèÈß?ߧØDVÇ?´Øð³N$?à,ú]Ԝ?´Øð³N$?¼"՗C ?£¡l¬é'?ìm}…Mœ?£¡l¬é'?ÜǨŒ6ë¶?בfé²Ðf?áœ+¹äŠ%?בfé²Ðf?µèšiÀ?º¹Évei?í_]BÑ5è?º¹Évei?Ó`Â[s´?¶×'ÕfA?æOžÒyÆ&?¶×'ÕfA?p…x¿Í<Œ?d;<d/æ?ïÞõ=
/?d;<d/æPSR4FGL J2030.3-5038¿î?N\ââ–ÀB% …²À;MäSÒÀ<¾ßê¶ÂŸ@!üщÊï}?ú¶_¢ýÆj?È¢{1úy?«s¤i¡?ãè‹9"†@ñðÅûLg¿ïøª*s?ïý`t#"¿Ê;-½þR׿³½Øþ‰]a¿×(¹|ãÖT¿ÝáÉÿ={UNASNone?ïÿGðüÏ@?'o6WJ?á2)´–?'o6WJ?ïõ»z+ô?XRlD‡?T‰þŠvÉ[?XRlD‡?ïò	‰Zv?[ǽ2Ál?[ìí JA{?[ǽ2Ál?ïýÆB«1ƒ?Õ¤|ËYA?1Íì>'o?Õ¤|ËYA?ïÿ`²67c?ý8ïá?é¼!9×ù?ý8ïá?ïØLdÝzD?}4D:wŒ2?sÙ͔ò?}4D:wŒ2?ïô."¼5?ddBGiËG?Vý£a÷õM?ddBGiËG?ïù«Ëa?AayLJ‰g?IR³×¶"?AayLJ‰gAGN4FGL J2030.5+2235¿Ð;³À#yí9SÞ¤À;8
‡=À<'JŸ`ƒ@!‡'Kœ‹'?ð7`Sý®?àXBaNz?îLYµ@˜Ôw¼@.¶YBç[?ên^ýçKÿ¿ïñÊþ@9?ïþ
a'l)?pu¨ßÄ¿á'ïXèϿⓢt3®ƒUNASNone?ïø¡Q?I­°t7\î?O"õ°Å†Ä?I­°t7\î?ï·Ñ(.ÐÖ?DxTûYþ?'µüâÐU?DxTûYþ?ï¥Ý¿ä1?€lóñn`?†ˆ"&?€lóñn`?ï¤	§?‹^¶–qÊ?‹~ãZ¹Ò?‹^¶–qÊ?ïçÐZAõ?ló?¥vål?h/¥ù¾X?ló?¥vål? gÝ?±®ÊÝ
<?¤G=üãã?±®ÊÝ
<?ä¢ú?%NªCF?‹ÿÖø	œ?%NªCF?ïق"Ø?˜C$)ñd3?ŸdϬ]é?˜C$)ñd3AGN4FGL J2032.9-0005?ÞÈ"Îå'À6tÅÉ£MÀ;nãª2À<f©¢%YV@ºãÓNœ@{GA1M?Ĉ\ÛMC¿£¦8ŽfàŠ?ã\g	#•?øÃÆ0{s?ïû<aZ8¿è»¸¨Rš¿ç!Ë+âÜÚ¿àÏπÜ3r¿å¦v î?¸¦g¢0UNASNone?ïû	nœH~??¶À:†Û!?CÚEý^C™??¶À:†Û!?ïÁËýTª?†Šnça?{›r²Þ?†Šnça?ïÞ3~ †!?tc4g™¡ç?pæA
‰ãC?tc4g™¡ç?ïϗ‹ˆ›?\úzËc¿?x4:63 ?\úzËc¿?ï÷‡ˆ–ð?NLòäCúì?PñßFÈ'?NLòäCúì?î9ñï	ý?²·xG|?¬fðá`+?²·xG|?ïÍdµ"Õm?€OÍa4å?yM¥/eým?€OÍa4å?î^¯€ê(Ü?–ú?sHÒ ?ªóñ'@?–ú?sHÒ AGN4FGL J2035.3+0557?èŠÚöŸóÀÀ3ãêòQÂÀ:Ê°'Úb¸À<#à{Ö:@T­›"*r@͏ãÖÕ?ÄT±2<".¿ªÐû«©?äíò¼@®)Zvå¿ß²køvžÃ¿æ°ÕÀ'U'¿ïÿþˆ0»Š?ïÿÃÏÎ	
¿âgÿyÈC¿ðUNASNone?ïýt|ÿ…?V¡ÈØx?4\‹Dè\?V¡ÈØx?ïáïø\-ä?xr»WÀŠ?nn83Ï?xr»WÀŠ?ïÆÓëW°?¢TŸ…¿?|÷–'3ï?¢TŸ…¿?ïþÿ!]ȳ?…I%£³m? 
ê}Áë?…I%£³m?ïûy"À†?Hüߌ<ò?B톒–?Hüߌ<ò?ï9}AÊ$Ò?¢Ô|R7º"?˜ÐWÊ+Â?¢Ô|R7º"?ïZې+~?Œ3:î?Œ)Id¼q?Œ3:î?ïõ¼P"'?V‹&ÛÕ2?T‡_BŒÇ?V‹&ÛÕ2AGN4FGL J2035.3+0354?Ù\ég.¯¸À4÷Äâó¿À:éʄ0'À<Ii¦ŒÇ@âÝ¿
qƒ@(ˆÝ‰³s?Ç˂õ¾2«?™3èòŒ$?Ó5`F²?ýwVô-ŽÙ?ïúÏtFùº¿èΞÃO ¿ç§PÑÑ¿æI´´¨Ù¿ïÿæՌŽï?ïÿ˜ÁØRUNASNone?ïíãÝ#uë?]ëU¤þKÓ?b"Âm
x?]ëU¤þKÓ?ïÎ&NÑÒÏ?Ú*QÉ?xìع@Ï?Ú*QÉ?ïy•-VØÝ?ˆrŒó {?ÍZNE¬^?ˆrŒó {?ïÔÒ¤AA?_ùÌìG0?u–­È"°?_ùÌìG0?ïğäƒÅ?}YMŒmf¬?}°
µÞfX?}YMŒmf¬?îüٞ?­Â}Ëþ^?§ >ÁŠ8#?­Â}Ëþ^?ïuD]°'ã?ŽW՗F?'WtIí£¡?ŽW՗F?îÔžŸµ4?•æ%"D?§"¶¬Á?•æ%"DAGN4FGL J2036.2-0207?í>LõY¼À8/KøüրÀ:¿­FÈBÀ<dLÒJ»@}Š?©r@ï !·"?Ðx $Î?Ù{Tà2@Z&–m@Ý­)ï<¹¿ï§Ù}µ7…?ïÿáÍì¿à©ß'1.¿çôïËÕV¿ïÿõž}.)?ïÿxÃÐ¥UNASNone?ï!ɏ'¿? t'&H‡?›ÆÎ
ÈC? t'&H‡?î,©¢êë?´1¿ìÞ?­>%i@íM?´1¿ìÞ?ìXU¦«?¤ŽõE¤Àb?½=RËÚ¬?¤ŽõE¤Àb?î:†¦DDJ?'Íý¿×ó|?¬W•šßÔa?'Íý¿×ó|?ékn'¶ön?Ã-SÞW?ÊREõ$&G?Ã-SÞW?à>"}dž?Ó¡µkv	‹?߂Ù6Ã?Ó¡µkv	‹?職Üêk?²š—jq6D?Íù ŒVSã?²š—jq6D?âˆØtÜÜö?À-8TQ³H?ÚîOFF?À-8TQ³HAGN4FGL J2036.3+5642c?Ó«Æ2åì•@#Lµ»8PÀ:T˜ÜÛ7ÊÀ;ã·½q7@‹«(7V®@JNz·VC?О¿#@ø?ՈE^XûÅ@osۙï*@,ªžP8?ïÿøãú¿ÝòÅÅF››¿è6ÝâžÆ¿é@€Þ·°Ü¿ïGY•?å@\FQóéUNASNone?ï»!—æwT?~຦>?7šxë?~຦>?îÊò±Qµï?«(ƒe|eê?£PÔé,Ó?«(ƒe|eê?îX–E7}×?•Î9«?ªv›«¬;"?•Î9«?î*ùV P¶?@u`á3?­Pj¡j›?@u`á3?ïFë/tó?˜ÒÍd*-?—"š´s¨?˜ÒÍd*-?àغÁ²gq?Ò'™ísÙ?ÞNŠ|›1?Ò'™ísÙ?æ_•Ð§?¸1é8~¦Ã?Ó@Ô_×ð±?¸1é8~¦Ã?áiÝaÎâ?·Ø~ˆ{w
?Ý,E<cø<?·Ø~ˆ{w
 AGN4FGL J2037.0-2826¿ïܽ&!ãçÀA3»¾‡¬À9âÓì{¾½À<@xã@¬˜@ßÿÆÜH@âE¿ý±q?»«É᤹ø?½ÌR֑?þ˜ªX-¾@%ô†O:¿ÙlÿiK¿äsãýjúJ¿æay,;È-¿ëeØÂ#{…¿ãÈ:@¿ïÿCÂw‰NUNASNone3FGL J2036.8-2830?ïþIÓCð?#J7Ü8C?+bȺéŽù?#J7Ü8C?ïè0yþÊ?sޕúó?gÏå¡~;?sޕúó?ïÞÅ+Süé?r©}Ÿ`€?pjD#"Ö?r©}Ÿ`€?ïó7¼ýf?Cjzâؗ?Y†ƒ?Cjzâؗ?ïüq×1?<Útqž?<qF"ZÆó?<Útqž?ïyÔèؤ¥?–ñíëè>?Åbè[]?–ñíëè>?ï­<ÒÕ`«?†*R`‹`?"°Ë[Õá?†*R`‹`?ï»Þ;e?o4GŸÇ?_£TN?o4GŸÇAGN4FGL J2038.4+4212?yy=¯?á^wïû¥þÀ7çÇҒ¬À:6ÃákÀ@–¾Xéò@9Ó{<·@?·ÿvä܎?Ø+L'Œ@ ¤zž+Ð@‰ý¡O?èJ*Æ}'s¿Þ/–Æ€'q¿èHüލi‹¿éº\‡ÀSB¿îSfQÒ[¿É½‹¦¼Â¿UNASNone3FGL J2038.4+4212?Á$<¨Û^"?ÊÄ1'õ·?ë¶ðÕÉ([?ÊÄ1'õ·?±7ם5Z€?±¢vÙmr‰?íÙYT°?±¢vÙmr‰?ÑßÑ%;?¶{}EÛ>p?çqymc?¶{}EÛ>p?'Tæ8·4?~R×腢?ïm_0‰'?~R×腢?ÒO-ü"áè?אÛ.dl?æØiî?אÛ.dl?…dny?Í`ãž	;?﫟º‰Âü?Í`ãž	;?ųyÌl!3?´KªÍuÝ?ê"!Œä÷³?´KªÍuÝ?Mÿ}.Þ?…ã·Çƒ?ïÿ%™?…ã·ÇƒPSR4FGL J2040.1-3137?ësW9'ŠñÀAèAÝ!êÀ:¹Åԋ0À<<š	+!í@ÐõšKpA@š(»
,ª?Í徶3®-?Á·-[?îÄùdŒW@>½õŠ±?ïq¢"¤À¿ç]tàQ¹Ü¿æ 0÷ïF¿éÌòŒyöf¿Þ†õw/¿ïÿ°_ïÉUNASNone?ïù/Å{°â?RíIUD¼?K@êÈÚËÈ?RíIUD¼?ïÏm$÷]?†T–¢qÄ
?xInÀáV?†T–¢qÄ
?ïå[g7?Šy¾"uö?†¾¶ä¢?Šy¾"uö?ïá1øíßc?X

Oü ?nÎ!ܛ?X

Oü ?ïõ¨/So?`'=:6Gf?T¯÷óÏŒ?`'=:6Gf?î»VÉý?®[:a›h‹?¤J"n~°,?®[:a›h‹?în'#k¦(?¡_Ç,ʚ?©ÉEˆ?¡_Ç,ʚ?îå'yåt9?'®(ƒ*?¡¦è`ÌÕx?'®(ƒ*AGN4FGL J2040.4+0312?ÜlºáYÀ6jǸÕ¦À:¶Ø¦ãÀ<5Cu –
@ FKé¸k@A3æÉÎ?Õjpr[g?ÑëNB-L?þ×]I‡2@St^v­Ü?ài
à"S.?ïšÅ³Ó׃¿ãúz_l¢¿áÎjüÎX¿ïû¼~Ëâí¿ïò&ޑoUNASNone?ïirŸÚ¦T?"4¹H '´?'Ñ«ýËý'?"4¹H '´?î¯8váU<?©ÃËáTb?¥x'Å;?©ÃËáTb?ŒZ'$?"ø²³åØß?¦ö—=Í)º?"ø²³åØß?í½Â'¾X7?'Œ¸8)ã?²ëéŸJÆ?'Œ¸8)ã?íy‡'¨[ ?°¼Þ;ÎÑù?´3Ãiá@?°¼Þ;ÎÑù?è›ÇW~'^?Ìy¤¸îj?͐â¢b†?Ìy¤¸îj?ëºÒܲ?ª}3'–E?Á·§Ì7?ª}3'–E?æ'ÊS†÷?ºÎ¡£©<û?ÓÆÜkXò?ºÎ¡£©<ûAGN4FGL J2041.1-6138¿žÊzÖî‹ÀBJ»˜Çâ'À:²Ìœ%eÀ<žÙç@/å(
eC@_ÀY÷Ã?Âz¦r	?±¿ÃúÁ'?ñ
£ÇðÄú?÷6¡þ»Ý?ïõ®£¿ÕoX½ÜD¿ã$À™+¶¿äïþ®Ç¿æ¸ž¬þÑ,¿ÐÀ£ÿN)YUNASNone?ïüb
Ùo??5yËüñ
›?<ïªP2"Ÿ?5yËüñ
›?ïÍPHÈ?…°}"ŸÀ?yW±u¸þ·?…°}"ŸÀ?ïÛöû
k½?rXmºx£?r'çÉM?rXmºx£?ï¬öˆ‡ù^?hؕ9®éŠ?"Â]Ӳԅ?hؕ9®éŠ?ïòŸpâÚð?VSbÿÜË?ZÁÐe?VSbÿÜË?ïRUÝNœ"?¢H´G€O?•µDQµ?¢H´G€O?ïÈC¸çg®?ûñ
kT?{Þ#¥	Y?ûñ
kT?î)@¯âJ?•úÀL¢C?¯kòn&a?•úÀL¢CAGN4FGL J2041.1+4736¿Ò¼¬A®Z@¡QÙçgƒÀ8rZ¼8¨À;1hWØ.@˙>ªà"@ÊåN?°hÀ]ӚÇ?Ó*Y— @ /ˆTÍ·®?ûË°å"?ä¡þíÜ<¿Ñh–¾•¿á0³[â~æ¿æ*ü-¨…¿ë'€!£hпîmm¡n$KUNASNone3FGL J2041.1+4736?z'pÎõ?ŒÄN¦»·?ï˱ááv?ŒÄN¦»·?²Uûñ8Î?²èD~Ëg;?íµ@Øæ>?²èD~Ëg;?ÄàBF1ÎÀ?¯7"q²¿?êÇïnsŒP?¯7"q²¿?ÙHø"?"Ëææð?ï77¤±ü?"Ëææð?RœAK<?I 88dx5?ïö±ßOu"?I 88dx5?†Ï	/yv?'I
ë(s
?ï¤Ã"éŠ?'I
ë(s
?…U+@û'?rö=îÔݳ?ï«æ«E=¢?rö=îÔݳ?A‡'Tñ?2w¤îáŽ?ïûžœT?2w¤îáŽPSR4FGL J2042.1-5320?éwm ƒœòÀBãŸÂ¨†œÀ;RÂ}¾qÀÀ<·ä¼­šØ@ 3Æ 
aƒ@T@C¼î2?Ëd¢ÁáaY?"píÓ؄¼?Êg|;ôº?ýW
Éĕ?ï[}¾Ú¿æh/ßkµÜ¿ääo ÷±Ó¿â¢)?êPÁ¿ÅÚ»!ÿ"/¿çNV"uUNASNone?ïüzH¬9?HÐøÿ_ø?</ä¸;œ??HÐøÿ_ø?ïó¡É?\Í~9 '?X༲''Ï?\Í~9 '?ïéxþ%"?pÇtû£§?f‡á4´¤Ï?pÇtû£§?ïüíËõâ?%­vÛZ_?<Ëț?%­vÛZ_?ïþUŽ…qø?0‡^?¢P3?*§t´S?0‡^?¢P3?ïÓ4´Á?Ÿª6õ^?vvåò†x?Ÿª6õ^?ïîÛ5#?mè¬úcü±?a€$؛oÚ?mè¬úcü±?ïëÙ¼ýÕ?Y3Üû"ó"?d~&>⢥?Y3Üû"ó"AGN4FGL J2042.7+1519¿ë—Œÿ$À0F[¦ïÃrÀ:ÈLÃ'1À<a¸Š©@q®óñî@꟣žÖ?ÅÒVúb²'?±ÒH·©Ïó?î¿>¿Xp?ý%"GÍÊ¿ìà‡)T ¿Õ¼­šØ]û¿à}Tß«KÉ¿å@x`cíæ¿É߄_u±]¿é\_UÑUNASNone?ïûAMìá¯?>h²¯­?BúLj¸k?>h²¯­?ïÒ8°[ä?€ƒM}gT?vã§Ñ^
±?€ƒM}gT?ïã7Ü©þZ?o'½'Žž?lÈ#eín?o'½'Žž?ïìÔò¶?LTD¨WA
?cä+#Gjf?LTD¨WA
?ïèV{N?fúaã"»?gé©l?'C?fúaã"»?î–'ÿDæ†?±>`U?¦€	ùɝ?±>`U?ïђQÚEå?~ä\),dY?w6×
™¥?~ä\),dY?ï_Y–8*?†v"^´?"Í8ú¿Ç?†v"^´AGN4FGL J2043.3-1520?ìëð/
ÅÍÀ?sBí»ZÀ;"2.PucÀ<wìÔªà@ 2¯Øu@¼Iº^5??×£e_Ö)m?¹ÂH9€?åó s'õ?þLjKù'Ê?ïÃ[Ÿc6¿æ
d(ô¿åt%kÊSv¿Ü W xF¿èEÿ©þl¿ïþ^à`'ˆUNASNone?ïøJ"I'?K€êíepã?N×vwGh?K€êíepã?ïÕÂ)ä2£?|ø! £nô?uêóɦÖ?|ø! £nô?ïÔ^"«?{IãQD¥?~5Ð×Öc¢?{IãQD¥?ïdzÝ+ƒ€?_¥ Dwãð?|&o½ŸØ?_¥ Dwãð?ïêM³‰|8?h°Å¢?e²L'â`n?h°Å¢?ï&!Fœ?¤ƒM
%¸?›;×7-•?¤ƒM
%¸?ïE'y¨ž«?•lÔì5ZÆ?—O°Ç|Ž˜?•lÔì5ZÆ?îŜhGŒ?FÕ!fp?£¦9'[#7?FÕ!fpAGN4FGL J2043.9+2051¿ã¤zÄIùýÀ*ŽZݜ'éÀ;;øÒåÂÀ<«qøjàI@†å'Á@%Î_ª?єDuû°?ÝÝá<ps°@
e:í;Ø?üãô0¾å¿íÜiøÂ?ïÿ¨Â+‰¿Ú¢Ô`"ë4¿é\'!֝¿ïÿ×ñÃý?ÒDàPãUNASNone?ïc¥.Î?–W
'õhL?"ž^Ñô3?–W
'õhL?ç¹)o˜œÍ?Ê>Q$ñã?Ѝ­ ÎÆf?Ê>Q$ñã?ì¦çû§UÅ?£í¸$«"?ºÈÀ"ÅQÙ?£í¸$«"?ëŸ-€Ä$?¡\·`àÝ©?ÁƒKüïn?¡\·`àÝ©?ì–.oÊú?¸J"¿Š?»N|¨.?¸J"¿Š?Ä9)'§Êñ?ÇÐJv¬ëÂ?êñµ¶
D?ÇÐJv¬ëÂ?å´TÓ8?»H¯¬‡w?ÕÓܗVY?»H¯¬‡w?Ôõ³Ø¬vb?¹¢xï)æ?å…&©ÄÏ?¹¢xï)æMIXED4FGL J2043.9-4802?ï)Ÿw:ZUÀC$O"}ŠÀ:a'W«¸€À<Á#і`)@݀$¨€è?ûChjL¤ô?ÃOÜ÷'HB?ã"BwsÔä@ob?ùó:¥|¿ï±Óým©|?ïø®6Ý¿ÅUP~ó{¿äd­³,¿ïÿÆTǏ¿î‹EC/ÑUNASNone3FGL J2043.8-4801?̓LcŽx\?ÍÂf)Þ(r?èŸ,çaé?ÍÂf)Þ(r?Ô»y'Õª?ȌÔ"ùÍ?å¢C>÷•+?ȌÔ"ùÍ?ÑÔs$9ñ?²Nžç×?çÆmãw?²Nžç×?ÑÍ&€À?²"+†å?çuxì¿ ?²"+†å?ÂxrÏͪ?Ó,Š¦"?ëaãL•\?Ó,Š¦"?µÞ–CÞ?ºß}i^?íLD-ELT?ºß}i^?®á½<û=? ·Ú"á?îä'­,? ·Ú"á?šŽËð›î?ŽR¦ËCP[?ï+×tà?ŽR¦ËCP[PSR4FGL J2045.0+4202?ìÄìù½ñ"¿à£öíóŽÀ9s?VW$ªÀ:ujhS@ Þ8¯õ@ªõ&ˆ*?»ŠgbèÑ¿´y€žP¸?÷쩬6TP@ÂúÅX8?×îyZ^ñ'?Ñy þ'bÅ¿ìv_"$m¿çZ"ö¥
k¿Ø*Hiü¿Þâ^D)UNASNone?ïP--Ï`?«'´	{?5úXŽF?«'´	{?ïͅ€?'?Œ:î	?y=1yͳì?'?Œ:î	?ë¿@*E+Œ?°cÅða<á?ÁÿVëQÑ?°cÅða<á?ïã2(`
F?YŒ!Or¼[?lÍ×·SH?YŒ!Or¼[?í¿t`5[?¶~?y|>?²\þU'q?¶~?y|>?î#ûùé™?´("¯Vä ?­ÏBõk?´("¯Vä ?ì7®=Ñ­î?°,¹H?ó?¾BŽrŽ?°,¹H?ó?=•Èæ? (±ùëG?§DÌ*
Ÿ? (±ùëGAGN4FGL J2045.6+2455?ìŠg0÷³À&Sü–þµÀ:í§þàEÀ<L2Æü©3@0mUÃÖÚ@¬¤¾Éç?ƽRÜEæ"?úhDµw?ËVâðz§@¢‰,d¿êµ×ÙôÓ?ïÿH 荿臦†è½¿å"‡…¿Öû!sîf¿ïÿ⾦™\UNASNone?ïý—kÖ?'Éái{É?3G0ùR€?'Éái{É?ïå;wyš?rzE~Tè¼?jÄù[+ã?rzE~Tè¼?ïã3A(œà?t½Yrþo?l̾¾¥ðP?t½Yrþo?ïùt¹Ì{)?4<eÍË=s?J-sUò?4<eÍË=s?ïú°
|ä5?A–ØV¤Ö6?E?ÕnÇ2?A–ØV¤Ö6?ï[«‹DÓU?¥=5i?ñ?"ŠŽ†]m?¥=5i?ñ?ïÉáT2 (?È»‰dé?{Vô?È»‰dé?ïÝUŒŠ£™?fˆ+Lþ4?qU9Ñ{Ï?fˆ+Lþ4AGN4FGL J2046.1-1626?ÍE\ɍ/ÜÀ@Mz$‰LDÀ:n"B€À<~3Ѿ¤@<]ˆ¿?ÿÉ>¢Òþ?ÉÐ1[‰"?Ú`?»ËÈ@ÛÂ3×@®Â+ß?é:?A‰¿Ýc5ÄÝë¿Ó>âéĪ¿ålb©Ã]¿î65{âÏn¿ïüTyÔØ4UNASNone?íòÍô%g?³ÏÈÍsA¿?°i_°«?³ÏÈÍsA¿?ï
,:'ðU?¤ÄgiïÓz?žZx­¡õo?¤ÄgiïÓz?êÔ?£6®ñ?«€uº¤þ"?įs%D;?«€uº¤þ"?îBó9j|B?‹#—š÷ù²?«ÐÌfĆâ?‹#—š÷ù²?äoPH¨÷l?Èÿè÷q*?×!_n®(?Èÿè÷q*?è¨(ƒŠl3?ÌWû²…?Í_]ñÖO5?ÌWû²…?Ú.{èG–[?»œÐŠ
t<?âèÂÜ4Ò?»œÐŠ
t<?蜵ÙHä©?±»ö~.¸?͍(šÜm\?±»ö~.¸MIXED4FGL J2046.9-5409¿Ê¹?Yå­!ÀC3֝0'À;+m,SE!À<²ãô0¾å@ ìôèâÄ?úÏ÷>^‡?Ô'Jœ±Q?ΨZè	?þvÜG©ã@~õ&`è¿ïUtÁrüw?ïώH,¿|¿ãto=¥}¿ÒæV
ΐ¿Öz±!µR¿ïB¡YºUNASNone?ïüŒòͬ?0ž-}Ì×?;›òpŠÎ¾?0ž-}Ì×?ïïcMe†?eò¯~4?`œ²ÓÿRz?eò¯~4?ïÉ®Éèq?z°ƒ9‰¥7?{(›…z#m?z°ƒ9‰¥7?ïòÁ=0s?Dü|(lîR?Z|္q?Dü|(lîR?ïüåÚv?8í&¿èù??ÐÂÁǬ?8í&¿èù?ï¿1.SØù?töïWˆŸ?€3´_³ã?töïWˆŸ?ïÑKP»ž?zƒ^C(0?wZ}jàÛ?zƒ^C(0?9žÃ?tÑ'˄!?€ÙŽ±!>?tÑ'˄!AGN4FGL J2047.5+4356¿ã9pÜX}?Ô7.À\ÑèÀ8ÿ,íiZÀ:Tù]N°@"§âÅÂ@½Þ½ç?ÓÁÚ`3F~?èæÙóü¼@þÓr&Ž@²aôçž	?î_u`Õ,î¿Ôjãêv¿íÛX¡ì¿ç"¸+U`¿ïÿõÿ 1#¿ãL?bUNASNone?Ýÿ°ÕK?Õݑj??áq§¸[?Õݑj??×û–ý̹?ÎÜ*ÁRMÞ?ä@4¤?ÎÜ*ÁRMÞ?ãözú-iV?³Á¶¦7?Ø
¥-T?³Á¶¦7?ÖËÉäÝ\?²H¶»ßæ?äÿš
'R?²H¶»ßæ?Ù0-¶,Þl?Ô"9L
/ú?ãgé$éÊ?Ô"9L
/ú?¦åê	7?·¿rµ,W?îžñ¯|§=?·¿rµ,W?Úá)ôxÀå?µÅ\ð¢¾&?âkߎ?µÅ\ð¢¾&?‰Ò.3å¢Á?w­A5ZM?G.%?w­A5ZMMIXED4FGL J2050.0+4114c?í;ÓNd^¿ûá>ß8àÀ9VN>QtgÀ:÷b§K3@ˆèœa@s¾Ãõ¶?È?m©%Ó¤?ÍHMv«X@Ǡʃ?ý+Vøà&?áó!R¶¿æK>AÚ
¿ã-ðžc,ö¿æIWÍFoP¿êUÒÀá|¿ívYùp™ÆUNASNone?îîÓ=1íA?¨S!EbW?¡Ì-½ö?¨S!EbW?ë%w5
p?ÂE\G?Ãj#+˂A?ÂE\G?íPÓzTÊ?¤ø:¶J¯?µ9eå'±?¤ø:¶J¯?éf¸52‰7?¥Y•ƒÆ"Å?Êe+5Û&?¥Y•ƒÆ"Å?àߛ)=ø?Êw5mÂr£?Þ@É×­"?Êw5mÂr£?ש¾fê¥?Òk5ý4k?ä+ ÌöŠ®?Òk5ý4k?â&Ý÷]?¸åìó!¹þ?Ûï²EôF?¸åìó!¹þ?É2…ê¡Z>?ªK«2ÊâÐ?é³^…W©p?ªK«2ÊâÐ(MIXED4FGL J2050.4-3015¿Ã©yÒµ3ÀBÖxl"h
À;þُRïÀ<€‰Ù25Ý@¼N¡MÃ@³˜Ôw¼?Ñ{nOê?Öbºà;>š@¤³ÃçJý?ý²þ½wÅ¿ïÒ·ÈXÉÆ?ïÿLa¢—¿à'ÆN-Š}¿éѼ ¯¸j¿ïþªà"Ô?ïõfI
5
UNASNone?l͑?‹Æìå¦Js?‹[\+À?‹Æìå¦Js?@gú?±PÿÉ÷?¥?F<Õg^?±PÿÉ÷?íc•8rC? ,èž
ï?´ãV>¢"m? ,èž
ï?î½îŒÔÔ?ŽçÁ
ߎ?¤.AÆg½?ŽçÁ
ߎ?îj©
óŒ?¨Z'hj?©UoN:¢H?¨Z'hj?â³Ä''?Ón®L6Âè?ڙÌwðÚý?Ón®L6Âè?ë{ÓXŠ¹5?©zJU?²Õ.?©zJU?åõýjZ´?¿Î:íß
?Ôý+J˜?¿Î:íß
AGN4FGL J2052.1+5539?ç|€Î¾áÊ@móùa€À:¹‹U38<À;ô×°´h@ös%@vÅ#‹ƒ?Ðt4…Bʀ?³DS§?éŽmìl¥?ü/_"K|?ïìFD‡ïM¿â¡DˆÆ¿¿êŸç[ÄKõ¿ÔÄ5N–f¿ÞÍg'ߐõ¿íäñ@õh¢UNASNone?ïøé{·¹ô?b`¼âتŒ?LZB¡-Ë?b`¼âتŒ?ïÐ,åU­?€–€Ëœ?wégÿ
'?€–€Ëœ?ï×Ò"æΚ?s°¤\
7?tî{j¦ß?s°¤\
7?1å´éñ?cÖú›7¹‹?€Û†"¯Û?cÖú›7¹‹?ïîôA°Ïk?`®|£yõ?a¾É<o?`®|£yõ?î(aóåë?°Ï]җ]?¦-yß	ÓM?°Ï]җ]?ïFCjÊ?G&ÉÝ?-ô#
Ä?G&ÉÝ?íá;œì½â?ž"Ž@A?°ö#u÷ó?ž"Ž@AAGN4FGL J2052.2+1635?ã æÀ1dô!-wÀ;
Á$"À<'=¢"@rò»ÉÅ@UÛpÔ~?ÖÊð¿\£?ïAÊsbÎ@Œ¿ôw5Â@†  ´k¿Èž&܍µ
¿å²¢\·¿áŸ¸Í;‡–¿ïÿyB=K?íöÛ>)±T¿ïþùoÃzUNASNone?ï–f·w®–?v|°5°?ŠfR,c.z?v|°5°?î™é¥öt;?·i3•Á×?¦aežàîQ?·i3•Á×?êߧH6ƒ'?¬
mhÏ|s?ābß%ób?¬
mhÏ|s?ïæQIÒ:?h+å$Ÿ) ?ip®¤OÎr?h+å$Ÿ) ?í	'khˆ?Àńë'?·³ì©–A?Àńë'?à®"S{Ê?Õ<"д¸Ú?Þ£èÙYk?Õ<"д¸Ú?å"s(Ý?¶¦L9ÒO<?Ô÷Á®G?¶¦L9ÒO<?ì†ãn¤ÎV?¼±Ð5üªû?»ÈäŠÙP?¼±Ð5üªûAGN4FGL J2052.3+4437¿ï'Ø=Ýö?¶öԈ-
¥À9̌5-À:¯
•øÛ@Ì7Ž·"@"rä#*§?ÅÃdCK"8?Ý»ÐZöƛ@µQþÐU@<""†âÞ¿×°Ôßøà¿×¿!='\¹¿ç*7Á¸F®¿íÂÝ_¿ïÿºà¼ô¿í¦.}kæƒUNASNone?à¢Eøæ8â?ÍÁ˜Çb?Þ»t3Ž<?ÍÁ˜Çb?ÌTZ•wËé?Ç&ýx	Ò?èêéZ¢
?Ç&ýx	Ò?âãpÛ4n?´SPó@1§?Ú9I—"Ç?´SPó@1§?ÕÉᣧ9?¯`QpØR?å.,tc?¯`QpØR?±i±Ñ?´-Yœ¬Þ?íÒÜ¿;È6?´-Yœ¬Þ?–¡ÐúÍÉÉ?¢_öì£/Y?ïJñxRÍ?¢_öì£/Y?Á(ˆ__Œ?¬_Á5Úë?ëµÝè(?¬_Á5Úë?ˆnÖ>¾ì4?u³´°õÎ?ïžD¦Î
?u³´°õÎMIXED4FGL J2052.8+5739?ä~¤Põˆ@  ¦°)(À:ÉÈ5ŽWÀ;Á¡ùºk¡@	ý½/ ×@-°ê7?Ä驼ÒXÓ?½½Šåv¼Ë?úB¾ÁqNø@V¦í•?èç$œ—zÛ¿ã¥jÞR¿é·à†=¿Üœ›PÓØ¿ëùoÃzn¿ïÿÚ €UNASNone?ïۉ)E.ï?o\ÍÂj˜?r;kHÊài?o\ÍÂj˜?ïyæ¨ëò?"!C7¼?Ã*àÉñá?"!C7¼?ï?«¤ç‰?Kç?˜
‹\/¤à?Kç?î·1ÑD'ç?'…Rcqä?¤Œâçk^ž?'…Rcqä?î´]çßM?¢Yóz+WV?¤º!}Âè6?¢Yóz+WV?뎸V7?ÂK›‹Œ;?Áŧ#ߝ?ÂK›‹Œ;?ì
!'S<?°4=anâ?¿Ï®öÅf?°4=anâ?æcÝú¾ïâ?¯âD&4B?Ó8D
' <?¯âD&4BAGN4FGL J2054.1-4054?äJ_!x ¦ÀCö FÇd®À:A…ô¡'À<_Öq'<Ô@´6"¦É@"*ú?¾!-¢$­‰?©s€Û¡k?낎»F"@n_.8Í?ïW¡!MW¢¿å'"¢‰­=¿çÞDÄU/¿áwáî-¿ïær$àŠ¿ïÚ8?ânUNASNone3FGL J2053.4-4052?ïÉKnF\?Ðáåù&?{ZHýF%¢?Ðáåù&?ïº3SÙ4Ô?"€
HС?s+€þò?"€
HС?îÝö*'ú?—œ•ˆ¤%?¢.™è4a?—œ•ˆ¤%?ïe·Ðnö`?~õlÑ	?"IéŠ-ý?~õlÑ	?ï@Lµª
D?£˜.9?—öiE—MŠ?£˜.9?îp¡ ¤$ã?±'Tà-Üð?¨õåö™˜Ñ?±'Tà-Üð?îéstýê?˜¼;Xf`—?¡hÈ­ª>?˜¼;Xf`—?í=ǵA?£¸^ª?¶ÂUgŸþ?£¸^ªAGN4FGL J2054.2+6904¿è}æW.Ý[@.'ÄupÅÀ:Lµ›Wß»À<Eþ7¨ã¹@&˜®²@ç~äâmH?ÂF­¹a5$?Øó;Ì@ O‹XŽ?þo'€EŠ¤?è(wŽ'ÿ¿Ä®QM¥¿Ý·A 3fµ¿é'Û¿®×¿é"'?h¿ïÿƒ9UNASNone3FGL J2054.3+6907?áâøÒS
]?Éâ¡WJŒ
?Ü:[YåF?Éâ¡WJŒ
?ß©®°é'³?Êâÿ
®ý?à+(§‹l'?Êâÿ
®ý?æ>¥'0|?²Ütø÷äX?ӂ´ûŸÉ	?²Ütø÷äX?äPþ"Í&0?¨ÈÿcB³?×^öe³Ÿ?¨ÈÿcB³?»ŒñCéR®?¶«{%\¨D?ìŽaׂժ?¶«{%\¨D?µú·ì•êã?¸[žštì?í@©mB¤?¸[žštì?ÇæÎ|`‰ê?´Ò.qP§?êL`ç݆?´Ò.qP§?¾'†¤ëÇ? ˜6§/&?ì;+}B‡? ˜6§/&MIXED4FGL J2055.0-5218?í/MܒúÀCèA¢a¿8À;>$'ýuÀ<‹î:ތ@¸ðá©þ—@ø&"»?Õވ¡y·Ò?Ñwûd9æ?ú«~3Æ@؋`pÙ¿é'Æýó¿½8¹›¿åãEf­¿âÚ
ݹ.4¿ïþÚ0bž[?ÏJùãÜ2ñUNASNone?ïù¥­ùøÕ?RÎÊÔ~5?IiH.,@?RÎÊÔ~5?ïõY1ZÒ?Z°'[È5?UMRšÜW?Z°'[È5?èDç*?†
²_½?Ýü"¥‹?†
²_½?ïýX	E<å?"àj«õݬ?5?¶sSÅf?"àj«õݬ?ïþ·CVI–?0wãïa€?$‹ÆÚmy†?0wãïa€?ïÕU™(tW?}Œ½ÅHK*?uU3qE4a?}Œ½ÅHK*?ïW K £Š?ç(£ùt?•ö‹ëŽ·?ç(£ùt?ïð÷^Q^?Rå4S—øG?^DLsó?Rå4S—øGAGN4FGL J2056.4+3142?ï«'!=M¥À!£;u!MÀ9<›õšKÀ;»¹&&Û6@웺Iì@]!ê5"?µðR

ú?ÚÊd<Àz¯@ ì'éSQ@gŸÜ~ƅ¿Ô>$ކ³Ž?…¤éó'ù¿ä-–¦ Z¿è±càO5¿ïþ®û*®¿×']<9UNASNone?Ï()'_>?¢ò¸&Ÿƒ?ï¸Ã_)Ÿû?¢ò¸&Ÿƒ?·þXâ6™Ú?º¯¼p´)?í4ãâh?º¯¼p´)?椙ýŽ?©¿¼h݁S?ëVـ\?©¿¼h݁S?´×›`WÔ^?›Éë?*l£?íe"Ùˆ"?›Éë?*l£?ŒÅi?¶IcM´Z?ê'ÁŸ?¶IcM´Z?•fš¯<oÒ?ž9{qœl¶?ïTË*O"Â?ž9{qœl¶? oö¼m*¼?–f†Ì×Al?îù"FëÄ?–f†Ì×Al?UµR96g?FÞs±d?ïõ%V¯AÕ?FÞs±dPSR4FGL J2056.4-5922¿æBi÷ë_ÀCp¾´ .À:]¹À€Ž0À<yµIc @˜üsÙk—@Ý_á'?Å6ò…n"?ÉOJUŽ§Î@¢¢&0@u@ãJÇ?ïòÏàþ]¿äøŽ¼ÆÅL¿ã"xKtÈ¿áÄ x°ëÆ¿ïÿíöé	¿ælQaòc_UNASNone3FGL J2056.3-5925?ïµì×ÀW?£5ýÂL?'"Éþ¼3"?£5ýÂL?ïç%ädˆ?n‡©3òŽ?hÚùü5?n‡©3òŽ?ïe}.˜³"?Œð
# iÎ?"PZ0Y+n?Œð
# iÎ?ïÂ2º'b™?bÙÜu¿#?~æ¢Å=™?bÙÜu¿#?ïSêÉô?Ú$¦"?Ÿ'¨yKê?Ú$¦"?ﮀY4W?CòAR:?"|é²ê+?CòAR:?쐺´¶?¨ÿÉËþî?¼z*_òP?¨ÿÉËþî?î±ó>jb¹?ŽQ¸ Ƴ©?¤àÌê8s?ŽQ¸ Ƴ©AGN4FGL J2058.0+3338¿ÒaÖÙ.ô¤ÀU´$_ZÙÀ;-¶Œ§—À<¥"²È@ƒŠ'3õ@-@«?ÏíŒàΌk?یÒÁƒmˆ@	.<b'?ÿüW¯>q€¿ïÿà iA?ï¡ 8Bg?îN™á=@¿âåÃ=×Ñä¿ê³"¢Ú¿ïæ^£úE¬UNASNone?îìKÏ{»?ª'äÙ*u—?¡;C
âIE?ª'äÙ*u—?ê6`J~º?Æìéò;`?Ç&~Öû?Æìéò;`?íÞôŽv"¡?áÔÈy?±[Ž(ø?áÔÈy?é@BÑÇï?ª$šád«É?Êþô¸àB?ª$šád«É?ê¼æϜ#Ñ?¿é¾×ãù‡?ÅdÁp»?¿é¾×ãù‡?á¨sbUé?Ó6ãÑ÷,?ܯÕ;T.?Ó6ãÑ÷,?ç3Úç±nf?¸‰ŸÀ¬o?јJ0#3?¸‰ŸÀ¬o?Úz	"ŠæÆ?À&ì¼4ì?âÂûnºŒ?À&ì¼4ìMIXED4FGL J2058.5-1833¿èRT—ö›ÀB¨ÁTɆÀ;÷sI£¸À<Ý1=­ˆ@%% _Š?ôÝWšÉ?ÑÇ"¾Æϳ?°U2a|Ú?ÑwÂd$ö@j&Õ+ëì¿ïÿõMõVY?ïÿ2æY¶¿ïþÛ½«q³?ï÷݇/3Ê¿Ýí¤2϶?¥'mœÕRUNASNone?ïûÄDåã?{ð¸ÞZ@?@ï¦Þªš?{ð¸ÞZ@?ïê•Ñý§û?p'moŠøz?ej.×e.?p'moŠøz?惘3`T©?…"‰iaÄ?…^s+Zq?…"‰iaÄ?ïüïÜ59b?2à†.U|?8 NÜ?2à†.U|?ïüÈC?	??v7›Z??q½õl`7??v7›Z?ï" ,µœ?"¯"?®ó?‹7ôÈpE?"¯"?®ó?凞³0¢?‡¡+øñ?…Ú">H«?‡¡+øñ?ïòļÃË?^ôå9œ?Zv‡mŠ®?^ôå9œAGN4FGL J2100.0+1445?ì=-;¼2À3üæâ!ȨÀ:ŒÙ™cé´À<@HÊt,ù@ç®Tçî@…¢Ëqƒ?҄‡ƒí_ê?ß5ÿ–Mµ@È§¤X?÷̧¨.]¿ ÊŠÛÄ?¿àåê«%)¿æ÷çÝõ>0¿í'E.Þ:¿àèú}	@?Ì$ZR[ígUNASNone?ïkprGµ?¾á³Å{?'œ1öÞs\?¾á³Å{?ê‡G@¬¦?ƽÐc7æT?Åââÿ¥Mh?ƽÐc7æT?îzž«™Ó?–Òìw4?¨VKÆÆÜ?–Òìw4?ìäÐvqî§?žxþ WÄz?¸Ù|MLqÅ?žxþ WÄz?ï­Óö•P½?FH¶=™]?"‹a‹¨?FH¶=™]?Á_IW¥?ƒ *º5=?ë¨-¹ª8×?ƒ *º5=?éÛjY5?²"ê³<­Û?ȒV™¿¯-?²"ê³<­Û?Ñ0瞵7Z?»éFÉÄ/?çgŒ0¥dS?»éFÉÄ/MIXED4FGL J2100.0-4356?֗­˜v{TÀDŽDR?gõÀ:{®•ª ÐÀ<s"vD)û@¢©"P¯@Ì"û­Šè?Âă½B(?±äÖ?íÛ{@¾>?öÈ¡›@
¿å²À?à¿åN.â´G¿åCì>Bu¿â.'Z·Ü{¿ëŽ'Èê¿ý¿ïÿV"tnUNASNone?ïøPG&k`?R¢aD«~?N¾ã$?R¢aD«~?ïͦýìe«?‰÷E@¦?y,]Ž½?‰÷E@¦?ï™=Å´"?"P¿êGþ8?‰°Ž¹ÒÛ@?"P¿êGþ8?ïÂö¹ý‰¥?f»¿‡M?~"¢ôܕS?f»¿‡M?ïôˆ¢Æœ?]{Ž7Ûú?Vî»(vÛ?]{Ž7Ûú?ï"_@Ø7?©®X,ØÏ?›¼Á?©®X,ØÏ?ï$P?‰g
 ê€C?Œ?v舢Î?‰g
 ê€C?î iï?žôÉ
ãmT?¯ùskT?žôÉ
ãmTAGN4FGL J2101.8+5044c¿í–îïaw@½šzj)jÀ9ˆÁe}'À:Ø´«m×t@˜^IŒ¦@"¼¡Ÿ?Ñjþ;.Õ+?ҁõuü@5" ¼8@€ˆ'tð?ï¿ø="ßE¿ÕÔ~œéf¿ç|΀2À¿ë8–IƒÑ¿ïúmN·óø¿î2í"ñÚUNASNone?í×Svʍ?Ãc‡8>?±GÝdI«›?Ãc‡8>?ì|9Mâ­?º®ü'G—?¼5—ˆê—?º®ü'G—?éBÿQ}¹?²Ú70:QØ?Êô»ò	?²Ú70:QØ?ê¸5;B™?¢Ì'wƒO?Åï+õ?¢Ì'wƒO?æÐN¯îù%?Èw©ü×ñ?Ò_b "
¶?Èw©ü×ñ?Û[œ®vöW?Óc72‡?âR1¨Ä"Õ?Óc72‡?Ý1¬Ž"º?¼ƒð̪£?ág)¸ò5£?¼ƒð̪£?ϹõUhM'?°ò}©¥?è'ª¥ìŸ?°ò}©¥(MIXED4FGL J2104.0+4623?îpžÑ;òJ¿Ôj"m¸j?À:<»+º˜îÀ;¸–ªÑÐB@Îäõãq@:µå)»?ÏUöV³ëÕ?âVr¬MÑ@ó-¤}ù*?ûrA>¿åÜÁ6–•¿âiOBÇ%¿ÞKZÓ¿ènq'yAŠ¿ïÿÿ" 5•?ïðÔ^;Ÿ"UNASNone?ë̑§÷o'?¿¶éᅖ'?À͹`"Cf?¿¶éᅖ'?ç>°Ë̔?ÎZoÚzׯ?тŸÞhfØ?ÎZoÚzׯ?é@özù£ù?®f­-&''?Êü&p?®f­-&''?ëµ_õß?¨ƒ¸:%d?Ãå+ހ("?¨ƒ¸:%d?߆òr£¶~?Î2_£Ô†?à<†Æ®$Á?Î2_£Ô†?µz4öî
®?À'›MV}™?íP¹a=»*?À'›MV}™?ØІ÷fº…?¼ÁÖl¼Iz?㗼"L¢½?¼ÁÖl¼Iz?ͬ/ړ?¹<qÚ¿¨?è"ô>‰[<?¹<qÚ¿¨MIXED4FGL J2104.4+2116?é%íÙüyýÀ0ъeI/õÀ:cÖ1riÀ<3­¬v0@ &J4'æ@çÝÿú÷ƒ?¹¸‡E"©¿ Ëq>AëC?èÑÌ`–BÍ?û‡«¸°¿ïç:ÁòÔ?ïþ|ý׆º¿èktøÐ`Ö¿Þ±ù⯍!¿ß­j0öB¿Ø0~ã"õUNASNone3FGL J2104.7+2113?ïú禱žã?=µö»'
?Daeÿú°—?=µö»'
?ïÃN^p+?…¾›ˆf~?~Xøêäò'?…¾›ˆf~?ïév¥	 ?eî–Ã?f‰Z¾†Èº?eî–Ã?ïÂQnmØ?cýïÖNm,?~û×Gi;ÿ?cýïÖNm,?ïð­óÔߧ?Y!ËƁH?^¤Câ?Y!ËƁH?î,¾6Sp?¸j¯6Q[?­4™)5?¸j¯6Q[?ï×&é'«?{	‡éÇó?tl‹ŽÔòž?{	‡éÇó?î?§P͉?›Û®
@«?¬Šð"¹K?›Û®
@«AGN4FGL J2105.9+7508¿ïþ>i'™@2S^"ñÀ:+Õ£5#ÎÀ<8(¾e*ý@5¥›ÛhF@"}ÔA5?½#qõáõ?¨_¹<æÔû?î˜p9Mÿg@y®$û¿âßßÏp¿Þ)«|ñ¿æ~"4­†¶¿ÞàÙ>Ú[¿áíks¡R¿ëZsž³3ôUNASNone?ïù¶Å&2?;X3,5ót?I'°'ó¨?;X3,5ót?ïêŒÙË@Ž?eÎ$ÂZ?es&dÙùz?eÎ$ÂZ?ïíG-æî?bV«¾£T?b¸ÑöµÜú?bV«¾£T?ïůA:w?`\US_Æ?}¨fñè™?`\US_Æ?ïï_~AÏ?T&Ÿák+?` '<PÄ?T&Ÿák+?ïšpŽTäU?'<³Þ–H?‰cÜq¦"£?'<³Þ–H?ïÙÇ4e?z7B´H6?se´¸J‰?z7B´H6?î È³ž¹¥?¥VèÏIÅ?¥ótÀ°°?¥VèÏIÅAGN4FGL J2107.5-1507¿ê'#Ë®ŒÀBn;ÑgfÀ:ø0ÁhëÀ<2¨J6"÷@ ø(›)½@՘ZÕ8¬?ÂaÓY®Çÿ¿»¹f®_Ï?ýî}÷|¤?û}/և`²?Ò¬æ}wúã¿ë¡É¿îZU¶ë¹ø?ÛlKU‡¿æOËàÏ»¿ÃàS<h5UNASNone?ïÚ3.šÈ?«˜J…§x?rætx€ÏÞ?«˜J…§x?ï—÷¼uÍÉ?˜d:AcZj?ŠßñØ?˜d:AcZj?6g<?‹°@¾Ðπ?òbÁ<â?‹°@¾Ðπ?ïçJ^óÖQ?`Ž&¦·T?hµ¡I6õ?`Ž&¦·T?ï×øš¹‡Ô?}"õ}æú¼?t²"Oš?}"õ}æú¼?낛¥¯ÉÔ?Æ·Æë·H¬?Áõ'i@Ø°?Æ·Æë·H¬?îuçUf?¡–Xù>»j?¨¡†.ûž?¡–Xù>»j?î ð%?¨bYǘ?¯5ñBKþ?¨bYǘAGN4FGL J2107.7+3529¿½Ø£ðŠ—À A_ˆü"dÀ:~¶H&	À<
ÿÖ"î@P@".þñ@È"ä0–¡?ÈzyBáüà?¶ÖÖ»ãñ?ó"Gö8Öá@  BU:?êDã߸⵿ٍDv§|¿çM}ŒGÌ¿ì	áàÛ!¤¿âƒŽ_©³Ã¿ï«a]*UNASNone3FGL J2110.3+3540?ïþ>:½?"
xŽa'?'Ÿ"?"
xŽa'?ïéք R	?r
Ò)¢¢—?f){µw?r
Ò)¢¢—?ïã\.1Ê0?f¹¸ÛÄv?l£ÑÒUWâ?f¹¸ÛÄv?ïûɄ:Y:?&p#€›?@Ùï8°ÒØ?&p#€›?ïúŽÒýN±?GvU´.ƒM?Eijàpr¼?GvU´.ƒM?†_?ŸxX
Àé¹?‹Üoöù?ŸxX
Àé¹?>?‹8¥Ì­Ã?ŒÝ;±'Dý?‹8¥Ì­Ã?ïí-œè¥é?Rþ‡2Á,?bÒc1w2?Rþ‡2Á,AGN4FGL J2108.0+5155¿Ýúø!h@N>ò"{À8í̙¡&VÀ:vF›ÅÃÄ@©PÑ~¸B@:ÙºñØö?À\‡ÀSAÆ?ÐßüÉï£@NÅ£ßâ@
¢›Jõ¿ïⶮ}Vm?t¼j¿âþÚÁW"Ò¿ècê?ú@ù¿ëòpK™¿ïõA?æIöUNASNone3FGL J2108.1+5202?ÍÂێ±‰?̓º"
?èzISž?̓º"
?ܱh÷Ôý?ύ&cìäo?á§K"z?ύ&cìäo?áð86Ó&?µ+¼cý?Ýâ'Y´?µ+¼cý?äÁ €Aó"?±¸àoŒ—ã?Ö}¾ÿ|ø?±¸àoŒ—ã?¢¨ÁÞ9å2?®±
4Èo×?îÕsâa­?®±
4Èo×?²ê†®R?ÀÔZ4ÔÉ?í¢¼Ðv?ÀÔZ4ÔÉ?´¬³•?Ù?£çD­
Ø?íji.Ɏ?£çD­
Ø?²¯G»1m+?¤ï(›?íªb؛?¤ï(›MIXED4FGL J2109.5+5238c?ÉæÁÚDHs@	ݜþ¨çëÀ9W"¥>ŠÀ:ÄXÉűP@]±°ç"ø@Ò¹ƒCì¿?ÆCß=g¿'?µžÃúì?ñݸ'#Zx@DgE‹%?îè¹AՍf¿å%nN'4¿å÷ìÀÞ(¿ç¸Û^
!l¿ìӄABÀo¿Ýޘ|84ÐUNASNone?YL]¸?'i8Ca€X?ˆVéŸ*"?'i8Ca€X?ﮆƒ}	?Š˜¶g'"ü?"^}'×Á?Š˜¶g'"ü?íãKµ-?¨#QèÐÅr?·ç4c?¨#QèÐÅr?金¹?¾ËÖÐUF?Þ‹u›`å?¾ËÖÐUF?íÖ_¸t?°c*¡Þx?±OÍaã?°c*¡Þx?ìóÎ	ýs¢?¿ðj÷Òd?¸a±^=j?¿ðj÷Òd?ëöUl¬?®N¢Î—?\?ÁÀ&«æMQ?®N¢Î—?\?è ™­æ'«?²—= ڂ?Ï}™HeõR?²—= ڂ8AGN4FGL J2109.6+3954¿ÒYÀgÛþ»À¹_í¦a(À:lf»ö»´À<PÍwí@"`´á¼©?ö)`F'µ?ț	›µ'À?ÔÜo×ÿ0@f}þ2 f@hH0p`:¿ïÿ&DÉ^?ï÷
ø{§¿îÃ`!¨Ç4?éìu:'Ä¿×C­¿@r6¿ÛªŒ[¨¾UNASNone?ï¿D9‹Š?¯î®íxÉ?€.ñÆ[}?¯î®íxÉ?ï§W\T·	?"Û9òÌ%?†*(çb¡Ì?"Û9òÌ%?ïA˜Ú¾
S?hS€¤æ?—Ìä­e¿¨?hS€¤æ?ïÝwÈõò?cªY7U¼?qDh\Nü?cªY7U¼?ï«ô~ÜBÐ?Š"øßl?…àL^çè?Š"øßl?îsâ²´•?¶îF"žµ¸?¨ÁÔÓÚDz?¶îF"žµ¸?îmM©^¼,?ž]›¶oª?©+%jð$E?ž]›¶oª?ï5ʉðc?"ƒô%]/ý?™F®Ï±¢?"ƒô%]/ýAGN4FGL J2110.7+5129¿ß+,Ñ;¾¿@ƒڐڮÀ98CEÏíéÀ:aÉí{ì@À•ý­ÀB@¬ dŽõÒ?ÐÏòñúƒ¿?ÚiÐ1Ü@
ïB-¡ú?ÿdÃo?ïÔ.öw¿à†h>ح׿èö=áâß¿í֎ín-¿ï÷/væk?ï²Û‰þñãUNASNone?ä=xþ»Õ?Տ±¹K?×ՅˆW?Տ±¹K?Ü*â½áÓ?ÐؖûÀ¼Y?áꎡ|?ÐؖûÀ¼Y?å­m2LGE?µ0,Gb"i?Ô¥%›gqv?µ0,Gb"i?â¦І7?¸o™íô²?Ûòz²^ó'?¸o™íô²?èë²s¹?Îkt–Wè?Ï«¤Q61?Îkt–Wè?¡ôVJ+˟?±''(&´?îປO"Ö?±''(&´?Ô­¥¹§?¶8ދ&"?å©t-#y­?¶8ދ&"?•ú½å˜™?D}'›y?ïP*Ž‡\?D}'›yMIXED4FGL J2112.5-3043¿æ3U}"‡9ÀE8Ɔ"ÄÀ8¹}'âïÀ;ûK¯Ri@æDÖ ³?ù?<;±'?«é³@pž?݁b ß9@1== ò¾Ï@'wVM¿|¿Ý¸çì
?¿ç¨eÜÔ¿ÄTÌ '¿àã|aO{=¿í/à˜[¬¿ïÿý±q&´UNASNone3FGL J2112.5-3044?hã)rüŠ?vo*mÜcX?ïçÖiG†?vo*mÜcX?¾ê¥®Xv?ÂÍ<w.Ï?ì"«J4ñ=?ÂÍ<w.Ï?¨ÞÆÁ½F"?œ®g™Ý°L?îr"ä+—?œ®g™Ý°L?@ú
¼$??»5‡ÀjÔ?ïûÁ}Þ??»5‡ÀjÔ?>,]‹§?¹&{Ï£#®?ïƒN}ça?¹&{Ï£#®?™Ê¡³ËG\?¥F…V/{?ï1ªòSçU?¥F…V/{?±bûÈcû?¦M:¼±?íÓ ]¸1?¦M:¼±>½Wjú@Ç6>ÈųQ»?ïÿüUE7>ÈųQ»PSR4FGL J2114.3+5023¿éUÊ5ۍ?òaKßÒcÀ9n‡–aÖµÀ:é×5Ü@£Dîq6@±3™Š€!?ÆÖáM¸E?ЫÈÛ¦"d@×"ƒ¸†Å@¥¤ªCàÕ?ïvŸ~µè…¿Ý[òú³åË¿Þˏ(ýO¿ãÏ¿®2¿í¾‹Ái¿ïÿ ß‰
UNASNone?ê&X}UÒV?À‹ù%£Ü?Çfž
¨¶©?À‹ù%£Ü?êÙ©ó?Á†{¼†P?ę[À3ûõ?Á†{¼†P?éºïã…Ôs?­égP/é?É@qè®2?­égP/é?ëÙ''{ø?šµ"TÌ?À›cbà!?šµ"TÌ?ÐA]ì"A?ÅQì56²]?çßQ	îý_?ÅQì56²]?ÔÁû»«Dð?Ð"á@C´?åŸ"*]ˆ?Ð"á@C´?׌]>{*?ºúýÙÒð?ä9Ñx`Âk?ºúýÙÒð?Øp"$Åå°?³–ùÁiÆ?ãǽí
(?³–ùÁiÆMIXED4FGL J2114.9-3326?֖oP£d&ÀE¬§?tŠÀ:Xš`hödÀ<QuÍâv'@¶²}k:·@¦¦Bˆ?½~ßrۄ¿â±†J‡?ÆÜô7Iî6@»Ÿ/Z·?êJ7&úƿ֔øà|-¿æZ*M±c»¿Í"‰ê}7¿åà• ãû=¿áÆëvÛÿpUNASNone?ïû$5`×S?7Ž	`=r?Co*r0²?7Ž	`=r?ïê7±"?qV§O¼`+?eÈN1j?qV§O¼`+?ïìkAÜ24?iþ˜®+†Ê?c"¾Q(£x?iþ˜®+†Ê?ïìâ'"t?J9ƒÁê?cn"æëw?J9ƒÁê?ïô]o`¥?Søú2L· ?VáE.ý&X?Søú2L· ?l V?˜ê1ì?ß$Þɳð?˜ê1ì?ïè›áX±-?v˜ô\û"ù?gd¾¬*š?v˜ô\û"ù?ïÇq@˜y?hõàê(ŽÓ?|G_ëÆÇ?hõàê(ŽÓAGN4FGL J2116.2+3701?éüŒ<'½MÀ ®˜ÜÛ7ÊÀ:"܅§tNÀ<=èõ!­@&*yPMö@ê#×u?ÅÒîNý"?ìZ0Fï©@"­`ûH?ùk5X'¿áF´"×j¶¿Òr‡[ÿZ>¿â7WOr.¿ì73"l;'¿ïígwžZ¿ïÿïXzUNASNone?±æ´¾?¾w|kéæ—?íÃ=©¦#?¾w|kéæ—?¾†KH¨»K?À3³(êb'?ì/6–êè—?À3³(êb'?ÒHƒu?²¶ä_H?æÛ·¾?7Æ?²¶ä_H?œG§Ñ™#ù?'+Þ­+f?ïÂÁŽ³À?'+Þ­+f?‹ƒ?,i)4?°§Ë ,ˆ?ï'ó\Ë?°§Ë ,ˆ?œûi®Ÿ""?¤
Bæ8ìv?ï$²o†ÿ?¤
Bæ8ìv?¨î	r{?š‹9ëšS?îqi²?š‹9ëšS?Anˆ6	?1—ú¥îð?ïû¤|)Ná?1—ú¥îðPSR4FGL J2117.0+1344?Í€±|uƒÀ7Þs×ÛõÀ:{Ì'‹_DÀ<Dô·ÍaG@²‹'Ä
6@=¢ø½ì_?Æ´©Ýßo?ÖÙ`®ìg@ìJ[mäà@ÃHïÝóç?íœK9¿áx¾'²!¿â<۝Ëœ¿ã¢–b­tB¿ì±–`)5ƒ¿ïÿÿ«FjUNASNone3FGL J2116.9+1343?î-aÖè7?ª#…\Ÿ?­/yäIJŠ?ª#…\Ÿ?î¸ã3@Ÿ-?¬À–€•?¤qÌÊ>?:?¬À–€•?íBìœÆ±?¢8Ô«ë
8?µèŸpôü?¢8Ô«ë
8?îÁèHö‹?'05…#'?£ï'xûO?'05…#'?æž·³—?È"&gë4?ÓԐ™üÒ?È"&gë4?åW
aò}$?Ðt– NB?ÕQë<·?Ðt– NB?ãCóc©6‰?¿QE}ô?Ùx8­'í?¿QE}ô?é$Rªz?­ôÞÖ?Ën·ùVº?­ôÞÖAGN4FGL J2117.1-5307?ͺфŽçÜÀE~\|ؙÀ:ˆL€À<'|»@ð–ºìû@	­þ«l*?Á¡ËiM÷?´®!7?õ­·þßn@o¥'(^?߬:›‡Z}¿Ñ¢[Õ¾¹¿æSþÕÞn¿ÑÆU#óпä¢n>÷âz¿ïÿ²gƸ·UNASNone?ïþ:Mâ>­?#¡Àã£?,[>KHg?#¡Àã£?ïõÑ;؄w?Y>YÇ"œ?T]‡ùÀÂ?Y>YÇ"œ?ïò9$¨‰?cÒ¥sÖ]8?[ÙSº-‹?cÒ¥sÖ]8?ïû¢‹ŽF³?&ÀAq×u?AuÒµž?&ÀAq×u?ïþºD¬NÊ? z[³?$[²*7Þ? z[³?ïÙ^Jãþî?|/ÄŠ?sPڝν'?|/ÄŠ?ïô>µa:?iQuì{Ì?W'"ÝV¹ž?iQuì{Ì?ïò̸k8?HºS?ZgÖpìÿ?HºSAGN4FGL J2117.9+3729?×DÚwQ½"À ŒFŸ¸À9žY …F%À;Ù ™hr@}xåÄëW@8J"xÈi?±«HÓ=?¿Téf`‡)?ûMÄ(¹\®?ñî¹Ç—¹?ßèGœÌ©ç¿áJ™¶õÊó¿àÙ๨¿åÉ£ý˝M¿íǍþZäR¿Ã·¹Õ¤6×UNASNone3FGL J2117.6+3725?ï§;aï¢ÿ?"!¨Ý‰|y?†1'€§¤,?"!¨Ý‰|y?ì<d{:ïü?À@½E¬n?¾Ü&(€?À@½E¬n?íێSã?Ÿq°£I¼O?±#fÅÝ?Ÿq°£I¼O?éFlÐÁW?¬º'lv7ú?ÊçŽL¼ú¥?¬º'lv7ú?êfWCÍy	?ÀbÒwV_?Æf¢ðÊÜ?ÀbÒwV_?Ú2V._äÂ?ѽ8
ý2Š?âæÔèÐ
Ÿ?ѽ8
ý2Š?êõb¤~¾¼?°ÒdEIÂ3?Ä*un?°ÒdEIÂ3?ÒoNûC`[?µr›Þ˜QE?æÈX'^OÓ?µr›Þ˜QEMIXED4FGL J2118.3+4055¿ê\	'âÀÁ)/»¯À;-î@ºÛ3À<j¦'F•ç@"OÄÄÂZ?÷eâ}8:?Ӟ)`ÌsŒ?Ó|]ž–¯?þm‹ÕÓÝ@úÐ<BüT¿î‰
€6œ¿ïÿý¡UûŠ?ïÅ!ò6?ïÿ"ÕåzC¿Ú×ÄØ6¸¿å[ח+*PUNASNone?ïûy8ƒ²°?6|X§Âbš?B‹Hô?6|X§Âbš?ïâaG·?x?êV˜Ž'?mžãôa?x?êV˜Ž'?ïÀ+ôÐvû?€«'ë|á?êŽÕ†]?€«'ë|á?ïï¡Ä?S©››&?`ÿ^"JÝ?S©››&?ïúw8âÕ?BÖG?Ñy?F#3ÔRŸ?BÖG?Ñy?ïwKØyK? Ûõ'<Ž?'Ÿj@¡? Ûõ'<Ž?ïÀųå?…Ç°w9nø?&
½ˆ‹?…Ç°w9nø?ïÔõÃå¦?rŒQ5hsÝ?u…7–~	?rŒQ5hsÝAGN4FGL J2120.0+5257?ïùÒg҈_@[©ßaúÇÀ9?踻ÐÀ:àF3À÷¬@SN×(›U@äõ$ÚªÜ?ÆF—i¾?艀qÕZ@"·þ®û?ö?ÊÎDò?ï}{áwÔ£¿×ïÈdÞ&¿áÅòÞ.t¿êûÒï)¿æÄþ;â¿ïÿùµc#¼UNASNone?ïZÁ'ƒ?žKµA2'Ú?"¾‡Ö׬?žKµA2'Ú?æ,å¡ZU?DZ¤nEA?Ó¦4½KûV?DZ¤nEA?ìq"šjé?¨þŽ--I_?¼sc,¨³?¨þŽ--I_?æœÔ–3¢^?«cHÈÈe?ÒÆVӘ»E?«cHÈÈe?é"2T‹‡?Âá}0àÑ?Ëw6¯áÑä?Âá}0àÑ?½
8cÚ×
?ÃjÑ|RG?ì^¸ó"¥?ÃjÑ|RG?ç2ä*%\J?´6ÆÎv"3?њ7«µGl?´6ÆÎv"3?¿ªÊ.ì?¤¬¯³ÒÎñ?ì
¦º>Ã?¤¬¯³ÒÎñMIXED4FGL J2120.5-0138?ïà"JäÀ@¾&ÉÀ;9'ôcê‹À<ž3>íÂ@!ÞdNß?þh7‹‡ˆ?Çh1ôo¿‰Û—.ʹ?ÃfýNÉ@$`Ρä¿îâÅÝo\Y?îY¨¿ãVöâv¿ÞVé†@÷A¿ÓÜ:¾l⬿ÌQü)ÝUNASNone?ïýÇùâ?&»Ä¾|^Ó?1Çi'1WÞ?&»Ä¾|^Ó?ïèþ³Ç¿?jÔ_6s
ý?gLqJ؅?jÔ_6s
ý?ïèߑܝ?p,œ²ÿúR?gí €ZÝ?p,œ²ÿúR?ïú(,;i°?2É1è ­?G_O´J?2É1è ­?ïû"ûO
§?=HÑUïØ,?Ct,="Ë?=HÑUïØ,?ï…G‡?"RÈ÷?Ž¸{ñØc?"RÈ÷?ïÞW¢rµ?|áÏϏ?pÔ.µ†õQ?|áÏϏ?ïämÀÅ$?aÍ	‰¿?k€'ƒó?aÍ	‰¿AGN4FGL J2121.8-3412¿Ýg–ÀFp(€QÉ÷À;É%,à2ÛÀ=*"¬ÊÎÆ@ £~‰x?ü—£U>S?Ú¥‹-lË?ïþáQ¿u@#È\$Ä?ý=ÓLKˆ?ï=è΋î¿ïÿõƒ¥;Ž?ïþìɹ¿Ãbý±@¿é3çcQ¿ïî´³ÑSDUNASNone?ê2u¸éÀù?Å´ÇI;n?Ç6)Xü?Å´ÇI;n?軦û	©«?Ì̑oç¶?ÍdÙYV?Ì̑oç¶?ë¿
v§/?©ŽUM!as?Á˚%cD?©ŽUM!as?à®'•WQ?¼'›ghÞ«?Þ£ÞúÕQ^?¼'›ghÞ«?æu½Fqÿ?Ð|gœ=Û$?ÓÏ…s?Ð|gœ=Û$?Ùjô5AÖ?ÔVZÙH?ãJ…·å_?ÔVZÙH?çlÂsW‹?·ýE@2y?Ñ&{PÞë?·ýE@2y?ÏE*	FƒP?Ã:÷õ&L?è.µ}®_,?Ã:÷õ&LMIXED4FGL J2122.3+7653?Ýöb-­Éc@2²IÂÁ±À:ù» Tž¾À<{:r•@0Fþl,#@£a~ ?Ëüð@šNö?Æô·7_?úk©f–7@ôÿý²¿ïÊ,¿%Å7?ïü% "Ÿ½¿ã[Š4¡È<¿ä®‹™%Ö¿ãÁöD•[F¿å™Ž´/óUNASNone?ïû¥?¥ó?7qɐڀ?Ak"'Z?7qɐڀ?ïç×F<>9?hü
Üž?h(¹Ø_oU?hü
Üž?ïã8óÖ?×?huìÖ)…F?lÇ6Àú?huìÖ)…F?ïÒu³ìâ?YÝÏ[ÎÚ?vÅ&¹{9?YÝÏ[ÎÚ?ïðÀÜËêÇ?Z5xø,T?^~F{hAå?Z5xø,T?ï|ñd©?˜çB˜ µ½?aÓx›CÔ?˜çB˜ µ½?ït¯¹¶?p"tŒP?'|jm­L?p"tŒP?&ˤa?'WeóÌV?¤Žú6ñ?'WeóÌVAGN4FGL J2123.5-8315?Óñ¸™äîÀ?$-òˆHÀ:ÍF«µûÐÀ<7™èsò@@ûEاK‰@¼Þ…[ôó?¬DµÝr¿£îî¾AÍ3?á3W{V@¾'$Ý¿ïýýÇ@›Ò?ïºa¤µ¬¿çÅä Óõ‹¿ãÝ}‰˜š–¿àì1¡¸¡ó¿à·Ð]óÑUNASNone?ïþ5²á·?$@‡GÙ®O?.L¤('qÑ?$@‡GÙ®O?ïõ³Y´?Z"®òl?UîÄöÁ÷1?Z"®òl?ïåFc¡?qÝK–¤í?j¹êÈç_'?qÝK–¤í?ïü,Ræ¤1?)
bgq9?>jÏ£·?)
bgq9?ïú)ü«,?EÝ%WêDj?GXܪ!?EÝ%WêDj?ïÓF^¼¬w?€@w±•ÎY?v\Кʌ¥?€@w±•ÎY?ïÎ&-Ľ?€Øõ		õ?xþlÜ¿	ž?€Øõ		õ?ïãDßiBË?c5µiÕA?l» È7"Ô?c5µiÕAAGN4FGL J2124.9-2433?ÙÚÿ1›OõÀEå.rÚ0À;sjZç­À<‰M DC&@‹/ûh@Eˆãhð"?ÒÞbKy¦?ž‡ô¼¼²?Å8L7;*£?ûB"°Ìf ?Ë<*'ÆÃs¿êÍø{§@K¿×úÉ?#¬X¿æYlÀd¿ïýñg¶È¿ïæÿ8mUNASNone?ï働͍?|ûÇR	Æ&?j|rÜ´S?|ûÇR	Æ&?ïÖ|Eö¯I?rYÐ]%w?tÁÝhP?rYÐ]%w?îÝÔ-p?"ñ°½êµ*?¢/â½AAþ?"ñ°½êµ*?ï®g 3wã?l‹àý;¤?"f8m9?l‹àý;¤?ïÚ´òÄ
å?p&"
 "ê?r¥†žªy‹?p&"
 "ê?ïDîÐ
w†?¢¹E	ä<?—b%üùAH?¢¹E	ä<?ï?¸|³°?–•ÌQõ©?Ÿ¸óÙ&?–•ÌQõ©?î]@Ýë®?•TAkrNX?ª+ò"üí?•TAkrNXAGN4FGL J2125.6+0458?×kò¬À>Ü@¿ã°>À;Në¯æâùÀ<˜%·I­É@ ü´fú`?ü‹Ë*5]°?Ñý6aé?½¬ ›$´?îƒÝo²@?þH%Ûܵ"¿ïÿúVrÓ\?ïþ½_ÇeÛ¿Ïe
gs¿Â%›¨±:¿ã3ÁˆK¿ÙZã¦XUNASNone?ïþZ'-û¢?#¼*'BÒt?*Vڝc£?#¼*'BÒt?ïØÑBìþ?€U÷;1ð˜?sø—~ÕÔ£?€U÷;1ð˜?ïÚðÉM³´?xيù­Pg?r‡›MwyÙ?xيù­Pg?ïß÷píÜ?U¬µEÀ«6?pt".õì?U¬µEÀ«6?ïý˜ãwo^?2<ŒFAÊr?38âI¥·?2<ŒFAÊr?ï?ž}¦k\? f‹5ŽéN?˜0IzƐ? f‹5ŽéN?ïãà27é.?tñ(]Lå?lÍý°¹¬?tñ(]Lå?ïsAØ´ÙÞ?ƒ!'	O!?'—ÄédÄ6?ƒ!'	O!AGN4FGL J2129.1-0240?ì™o{VÀAðuöý!ÿÀ:«åüjIÀ<=²¢i@ƒÉeeà@ÝäÅ©?ÈTí˜oW?´˜|c'í…?æÞ|Ý¡0g@	j
fEj?ï°~¿å±ú´f¤¿èf££׿ïÿ¬óéqH?ïût_ÎFÊ¿ðUNASNone?ïý-²b4Ë?v2N9OH?6'n$iš²?v2N9OH?ïìÂXC}?hÐaœTÚ?cè=âÕÊè?hÐaœTÚ?ï¯È¡Ñ:?‡ºz¤[Ë?"
ù̌ñx?‡ºz¤[Ë?ïÿßÅ^)½>ëÊv!Ïc>ðo7†h>ëÊv!Ïc?ïþ§¯u½¶?1‹QEMÐX?%…Ñ	l?1‹QEMÐX?ï–Ì`ã'?',ã|«f?ŠxÌàçã‰?',ã|«f?ïjÓ?z
Õ?ù`ö:)?'¥˜'Ÿ_?ù`ö:)?ïþ…ë֗?,%΢Ÿ?'¡EcpbÃ?,%΢ŸAGN4FGL J2129.9+5833e?ÅûäIb–ð@U›¡±–À8¯Û$~eÀ:Òe횢®@ÒqdFPœ@)Ưc/?³Hª~CQä?·˜¤Òód@ÏPB7²õ?þk‰0?ãÆ¿"9C…³*¿ÝÐ&^
§]¿æµV¬µ¿æéìb"IÏ¿äÒìnºÉ?³õR'AUNASNone3FGL J2125.8+5832?ïÔHëg}Ï?†xÅé¶N?uۊm=Xn?†xÅé¶N?ï?nmr'?œ6»["Ø?˜<·y%?œ6»["Ø?ëÉTgä(?«!D,?ÀÚ®cøo_?«!D,?í^Ãö/?™΂½0¹?³•	é*)?™΂½0¹?î{åKž¹ê?¥RȄ%¯‹?¨A«C€¬e?¥RȄ%¯‹?æ¶?ÜRÁ?ÏL»‹mA?Ó"€GZ?ÏL»‹mA?êp¼'…wp?³½}$Fñ?Æ=aê"@?³½}$Fñ?áïÃy^]%?»§1 £'|?Ü y
CE¶?»§1 £'|AGN4FGL J2130.8+2649¿v±W°³ïÀ1¤÷‡‹zÀ:ƒcj2£ÁÀ<T^üå™@8²yŠ@5!¬ˆŠ?ÖëU£öiÔ?Üýi¸*~Y@¢0[è^#?údW†¤Ÿ?îpï ´«n?ى+¶c¿æ˜ZRp¿íßø="ßE¿ÑƳãÇ»¿ïÕå¯ò¡sUNASNone?ïǙvÖ)?‹i‡78¾?|3*wã¿?‹i‡78¾?ë–ªâ?Âø¦'{?Á§—©Tw¦?Âø¦'{?îf‡6Ñ´y?–8-"'1?©—Œ',êm?–8-"'1?홨ª{
°?œS¼æ[ÜM?³2ºªo܅?œS¼æ[ÜM?î›þg	à?¬8ÿÙr*?¦@Ž†?¬8ÿÙr*?ÑÌy÷Š2?Ïl÷íÂL?çöÃ:ç?Ïl÷íÂL?è/sÈF!Å?µ{ýÿÚ??ÏB0Þçxí?µ{ýÿÚ??ß.}HwŠs?Â:á×î5?àhÁ[Ä:Ç?Â:á×î5MIXED4FGL J2131.4-1124¿ëîüú‰jðÀDN#c²WÀ:½T#mÃRÀ<aUy¯‡@cD¢œL§@¬Š7&?ÔÃmãæo?Û(mÀÍ»@9?l&™È?ûëg\…'û¿è…–½q:*¿Á¢Ú›¦º¿åÕ<Kv¿ëÙB[Å"´¿ïÿùJYQ?ïÿÚ@RÖgUNASNone?ïÃý ª/?€Ï§ò‡ý?~/¯þq?€Ï§ò‡ý?îǂ>Íßá?²WÅå%Ù?£‡Üm"é?²WÅå%Ù?íc··ðO? vüª˜Áï?´çÂAҊ? vüª˜Áï?ïoÿþc¯?‡wA<ü®¾?qÿùTR-?‡wA<ü®¾?îÊI Õ?¥ÿ͹³tÊ?£_Þëeò¬?¥ÿ͹³tÊ?â¾$fo?ÓjäŸý5ö?ڃ·Á3!Ò?ÓjäŸý5ö?ëióÊά?«ùéšË¹K?þX0ÔÅP?«ùéšË¹K?æÁŽ…
ã«?½V²iIE?Ò|âõê8ª?½V²iIEAGN4FGL J2131.6-3714?ïðÌÓµ,ÀG…WÞ
fñÀ;}ÁÅìßÀ<±ËY/F?@!B4éì˜?ÿ "•MÚ~?ÇB$½¤Ä¿¥µË\??âyÆ?"ë_@É͓ò?âh®_ybB¿âoçïhH¿äþîÝî³'¿â¥w=¤%d¿ïáÜÿI÷›?ïÀ­TžéUNASNone?ïòäO0¥ö?‹ûlÛ;º?Z7aF¾Å?‹ûlÛ;º?ïæãyë?u0§	hk?iéB¼¢7?u0§	hk?ïV¾Êÿ‡?hXÆû"?•(?G?hXÆû"?ïò«Ðl®C?Haiò´é?Z¨_—V©ž?Haiò´é?ïúNMu?QA(@_B?GÂÇU/?QA(@_B?ïRûú'?ž—ûl™òŠ?• œ©T³È?ž—ûl™òŠ?ï¥=X>õ"?‰;Ä5ÖN÷?†°©ðB·y?‰;Ä5ÖN÷?ï²3|aØì?yÕ~‰_E#?ƒs ñ€£?yÕ~‰_E#AGN4FGL J2133.1-6432¿ÛìØn|ÇÀD¤øßzN{À:Œv›gÐÀ<‡Tn^@tG]â‰?þ¡ú@£^>?ÀV9ˆý?äê^x[[p@r)AAé¯@0ì1A?ïü\ý†þâ¿Æ"œY½`ž¿ÕD«@5$O¿çŒ |aû¿ï"®"g³î¿ïÿÔÌuŽøUNASNone3FGL J2133.0-6433?¢õÐý(î?¯~Ùò÷š0?îТð/}q?¯~Ùò÷š0?Õ{>z9,?ÉŸ!?ö?åB`Âãiò?ÉŸ!?ö?Ĕñ9ò?­7Ûø.'t?êÚ܃±ƒ?­7Ûø.'t?Éé‹ýØ;?«ö^ñ›ñà?酝‰ñ9?«ö^ñ›ñà?p³ @vā? ;¤Ò ˜?ïޙ¿jtÏ? ;¤Ò ˜?·<q³ª¢?¼°0£¥¦?íqÉFœ?¼°0£¥¦?¤^"YfYÃ?™‡ü^ý? "#?™‡ü^ý?ŒleP^3´?{1}ãœþA?ïŽNjyÏ?{1}ãœþAPSR4FGL J2138.9-0408?ë©¡F»ÀC\ó^1
¿À;VÏj5þÀÀ<¬àŸèh4@Š ¹ˆø7?úC(ùôMD?Ý3ۀnÐ?æÁqðdx@Kݞ¬(@]wõ#¿ïÑ
ŸYƒ¿ã•Ð-hï?ïïñʳ¿Ö@›Ñ'>3¿ïü–ä•¿ðUNASNone?ï傹‹Úó?ž=cãª3ñ?j}F9ş?ž=cãª3ñ?ïØËmH¥-?|È>¡gŸ?sšIJ]·?|È>¡gŸ?îžVfWçŒ?•±lŸEø?¦™š‡:?•±lŸEø?ï~©Æ¸`¯?~ñ˜'Â<¶?*Ç1Šð?~ñ˜'Â<¶?ïê¿»[$-?l"¬'Ëf?e@DÇ7ë?l"¬'Ëf?ïvó®Ÿ ?—W¡a	?'=ÁS…é?—W¡a	?îÕZ,œ@=?˜ß+yIzÅ?¢ª]7ã.?˜ß+yIzÅ?ïP¹«Ý¿?—NÅa¨Ï]?ŸèÓN?—NÅa¨Ï]AGN4FGL J2141.4+0733?嘆˜vUÀ@6*Ã") À:…ì燫À<4ÛE5"7@kTù‹±@:aàŨ?Ãóʨku?°‡D­Y?ä¬é¢Æi?ú|=•âªÛ?ïÿtõubƒ¿Ûh(]lAÈ¿çì;AõmÖ¿æL,ÿ<Œ¿ïÿõEq#?ïÿµøtñDUNASNone?ïꢆäFw?wuVBP¸L?e]yÙ¶?wuVBP¸L?ï¨øµ;i?–[fL?…Áù– Á«?–[fL?ïZÒ?í¸?Š°ùS¤?"¥·û}'?Š°ùS¤?ïŒõ9†/?uN'•ò i?ŒÂ±¥Zì*?uN'•ò i?ï¾ÈœÞ¿á?€;v›aH±?€MØÙ&µ?€;v›aH±?íò´y*?¿Á°Ïk7±?·ØjZìԍ?¿Á°Ïk7±?ïö5Έ?"cÝA†€?Ÿ9]f/?"cÝA†€?ëèE³)?«F`ƒ¤?À_öé3"^?«F`ƒ¤AGN4FGL J2142.5-2029?îNJ,-`ÀGEŒÒ
ú/À;oA×:åÀ<ŸÒcÃ@ ´í6y¹ª?þñ#Xʜq?ÃN	M[¨¿'á´+ì?Ë2að
?ù\ò3Ž£¿ïÿÒþÀù?ïÿüÚ±'Þ¿áL	Þ¦%¿åÁ(ôëÏÇ¿Ëì쥿Ëiº¸M9UNASNone3FGL J2142.6-2029?ïüv"Z:^?5Š¿ÀyÂY?<Kd>{ƒ'?5Š¿ÀyÂY?ï嚐(p{?t6'û€?‡?jeoÄQ´Ä?t6'û€?‡?ï¢í4?þ?†É0¼ßŠ?‡D²õPȜ?†É0¼ßŠ?ï祥q
'?KÁ¼áG&?`We¿õÑ?KÁ¼áG&?ï÷¡Š‡`?H½®eEa"?P¼ëVóPH?H½®eEa"?ï`·çÒ%–?¡ýÌd–.?"éý$GL?¡ýÌd–.?ï¡Ðq
óé?ˆ	0k²Ê{?‡‹ãËuÀ?ˆ	0k²Ê{?ï£Öþ²?|±ŠCÀÀ?‡9
2"ïê?|±ŠCÀÀAGN4FGL J2143.4+6608c?Ê·ÚËΖ@#¿;ÉêpÀ:üíüÈ=À;¾X0ë@ÀU9@Þ~bÜn+?ÂÌv¦$—d?¹ŠÔø³?ödˆu"ç[@É2Vˆ?åguZ0G¿á~¸+¿ä߯þ_ìпêDùdŒW¿çE˜%%Sw¿ÅaŽ:jßóUNASNone?ïûà'6i?4ф[¤í?@cK/4"?4ф[¤í?ïãցßò?kêV8Y'd?lü)¬Ú½ž?kêV8Y'd?ïá²ËLw°?ffšãÎu‰?nM4ŠLÿË?ffšãÎu‰?留˧M?cچñŽ´¡?†¹
,×?cچñŽ´¡?ïë´ à¶?`רÀ?dKçJ¢e?`רÀ?ï"Û8S?¡ßi˜±#?›¾d'f ?¡ßi˜±#?ï+''•£É?•†ÒÒÏD?š»
K†Ö?•†ÒÒÏD?í­0¥9`?œ—Æ$º¯?·Ò–|Žþ?œ—Æ$º¯ AGN4FGL J2144.2+7709c?ïýX]'P@2.bÀ;y⏬°ÎÀ=6.Ú²@ #apˆSK@7#û‡Ë;?Õs4?¢­??ïþÑa‡•@òS—VÉ:?÷՜NÕ¦¿ïÿÿ&¦³?ï芘tÖl?ïÿ§ B€-¿Ô:©´™Ð ¿ï€]óÑ"?Ý+%þAcøUNASNone?Õ<¹ÂŒŠ›?Ï÷µº.?åa£¹º²?Ï÷µº.?Ø\¶íÅô?Ë-M's?ãõѤ‰?Ë-M's?㫗è‹çw?µG·ŽzÝ?بÐ.è1?µG·ŽzÝ?Ä5s>*?¬Ñ'‰xòØ?êò½;#0v?¬Ñ'‰xòØ?ÐÏ;fKŽ?Íòe3
?ç˜b|ÌÚ9?Íòe3
?³ÐWÖ1£²?µ8˞ȄH?í…õÑÊ?µ8˞ȄH?×}OC¨?½÷:…H:?äAX^«÷?½÷:…H:?—¿šVØP?'Ub1!¶?ïB+iÌ^?'Ub1!¶ MIXED4FGL J2144.8-1600?ï&)lWcŒÀF¾÷øËÀ;u¬QéØÀ<µ
qs	ã@ ¡¦a(9?ùú¡¡¥×•?ß;m>qÕ°?ÔrcÞ=?ø™&âÂØW?ûZ$¬1̬¿êï<-­¸5¿ë†®Š©<¿×¯•¤—y"¿ç°¹`´JË?ÍYjªmÒ@¿ïÿþR€ÖTUNASNone?ïñ}p\ù?]ûÄÏÚË¡?\åH]•?]ûÄÏÚË¡?ïâ]Rôø?x?ð†w?m¢­*¤P"?x?ð†w?ïN&¦ÝÏÔ?‹þYé~©ì?–;+%ýÓp?‹þYé~©ì?ïø4rß?Bf
0)Î?O/ûÌ@Ÿ?Bf
0)Î?ïÜíMG†?w¼3ɚa?q‰?Q,Í?w¼3ɚa?ïU0Ë`!?¡Mg{Š?•MùäÜ-Ö?¡Mg{Š?î늣:4ã?–»Ç/ëÖ?¡GUÎÒ?–»Ç/ëÖ?ïÂÇÓhÈ@?|¸Ýƒ´ò?~œ/oì?|¸Ýƒ´òAGN4FGL J2146.8+4808?ï|¹JJ7À}	@¢CÀ:oD"n¿ÑÀ;È[ז@FE}@¥1Àll:?Ç7ׇ»Ëž¿…ðYfE%Æ?ÁÊTâÛVþ@#J|ù{¿ØɁÿ-½¿Ü@ŸWs¯¿í±VNÁ¿¬Æ¡~Y;¿ì­×^v-?°žª`Í[yUNASNone?ïç ¬Íã?d§i;?h_S.lá?d§i;?ïî[ÿ
"?gˆئ€?a¤ü6c¬?gˆئ€?ïRE'H?$CGRz?•·MÕ8Ã?$CGRz?ïô¤GŸ?@tQ?#el?V·røg?@tQ?#el?îý…¢Ž,?¢°1¤|qw? /—¤û6=?¢°1¤|qw?ïŸþ9ë+?"wLô—š{?ˆ{³A>?"wLô—š{?î3ûãÚ>?¡,y\l¥`?¬ÀAÎ&u'?¡,y\l¥`?ïª3€ò?xÄ3¹!7?…s¹,&½?xÄ3¹!7AGN4FGL J2147.4-3854¿êPêõñxÀI\лnÖÀ;Ij­À<†,9
ä@!ÅX^è@ÈÈ@vÕ?Çãr€¦´¿Ÿåg}+"?ÕXTßd@IqŸŒ¨¿Þ¯¸¿ÏŽH¿ÞØs/Àã¿å!wI¹L¿ìŸÜßi‡ƒ?ÑÜ*7áïýeá±5mUNASNone?ïï÷õ£
i?naMԝqX?`
ÌÎg?naMԝqX?ïêŠnê€?sQ)ñ?eùuqy‹?sQ)ñ?ï,3üf?•z®"Ó³?š}9{F©O?•z®"Ó³?ïþîQE±ª?Íà÷"óÃ?!ë%ZJo?Íà÷"óÃ?ï͖°Óik?…|'¹ØS?y4§'Û®J?…|'¹ØS?ï^ŦÎò}?Ÿ…zR×h\?"'K-èS?Ÿ…zR×h\?î¯Ì5ošå?M],¶)c?¥<¦rœµ?M],¶)c?ïöYŽš?º?Q^Ö³Ùr?SLã(õêÃ?Q^Ö³ÙrAGN4FGL J2147.4-3713?ïÎô9£9ÖÀIðEwÙUÀ;=£_9MÀ<¥°<«'@Jô	Q¸Y@
© öÍ?ÔiÜÓ3?Ç(xY­ñ??ñÅÓé÷ÿ@)T ?ïK¤C@Çp¿á`<ZX¿ß£™!пå¸Úýgr¿ä°?bì^c¿ïÿþó…õUNASNone?ïìÏÏ6x?g†»vV"?c0û`äl?g†»vV"?ïä(¨.¡˜?x_Ù°"É?k×Wöz/ó?x_Ù°"É?B' H?†ùºQÜ&î?ˆÝ/f7&?†ùºQÜ&î?ïè4käÌë?M¿ކ?g˓ÿ¶5?M¿ކ?ïð
öQš?cI'ˆæ'þ?^ýäZÔ«?cI'ˆæ'þ?ïT}K7ê[?žåB"™}?•pVšº'¨?žåB"™}?ï2
ÌFj?"øûðJ?™¾F|Z&d?"øûðJ?ï¨Ùo"Úº?tdŽõy³?…ɤÉQe?tdŽõy³AGN4FGL J2151.2-4034?ÞÑü=ÀI^xB0üøÀ:ó'÷¾èÞÀ<£›€#¦Î@Ö7"¦˜?ýŽ]%u?à.ªØ†>s?ÊÖ¬Š2é?óŽR
}?üɇ5=úb¿é¹j"Ù5?ÑJ?f9¿æ(C ¾¦ï¿Ò<Š?3œ¿ìòs_ž <¿ïîövÛUNASNone?ïॱ¢F^?}}¥,×ÇÐ?oZN3zf?}}¥,×ÇÐ?ﮂæ¾F?˜*wì®f?"_FU‡˜|?˜*wì®f?î@÷Ғ'?œá¶ýŸ'?«þðg:ã?œá¶ýŸ'?ï£NHãHº?o€n 'Åo?‡,mʝmp?o€n 'Åo?ïÙU¤LP?}J>o€Ü?sU-ð…d?}J>o€Ü?î0Ño¯÷e?¸¯ÐÈm~?¬ò鉭?¸¯ÐÈm~?î©é"#Í? `ߤüà?¯¥afõ6? `ߤüà?îz"o'?š'0i‹Q0?¨V¹
;ø‹?š'0i‹Q0AGN4FGL J2152.0+4718c?ïþƒ7(òÀF¶¿DNÀ9®	SeØ¢À;À*zýÍ @öê5hl¦@
Þp?Á—ZúøY?Àˆb½Þ?ùÅށ*7@ՐÒÇñ?ík»9ýR¿Ý]Õ¾bü¥¿å {jÚin¿è>25r
¿è$SN[®¿âþ_
UNASNone?ï÷ñA‡p?Ho¼Ïº‹?P|¨Ôö?Ho¼Ïº‹?ïÉÔzɨ^?€šÆmÆ?{—I+?€šÆmÆ?ï¢:—M?­Z.0RK?‡qZ7
pG?­Z.0RK?ï"Ky¦	??z¼‹î;'?›¶É‡
/?z¼‹î;'?ïi~Bœ¡?"¡µÜk1o?'Ð-ò…Ø?"¡µÜk1o?$¬˜á?­F×´?3Þ?¦g¸¦
ì?­F×´?3Þ?ì8§¶è´à?°®/»"Ž?¾:ÂHºY?°®/»"Ž?ê¢å«?£å§*¥Ü?ÅtiS«£²?£å§*¥Ü AGN4FGL J2152.5-0607?éhóÆ`ÍÀEP|àP7À:ÎØÿ
6»À<Yÿu6@^X(`t@MYŸ®†'?Áí¤ž/€v¿»¾[T9"?ôáQ¿tè@ ÷TX?ïó×Ûôˆ¿é¾ÃŸ§z®¿é=²GæHŸ¿âçØVmÊß¿ïûDgõ?ïç!ý€É¿UNASNone?ﻋá*?«¿¢X4='?¸´#¢?«¿¢X4='?ïÁN6€?'wh"]N?qtsÇÜ?'wh"]N?ï>'¥áP'?'!bIwør?˜;HýW¬?'!bIwør?ïç¶2+¡D?Vþ½cæíÕ?hIÍ·'¡?Vþ½cæíÕ?ïµ6I›³?‹áH''¤?' 2iсE?‹áH''¤?í²^Bf¾?¼+¶Iõå?²m
í¥ö¤?¼+¶Iõå?ï=tđÚ?"¼?C´K&?˜\qeµöÎ?"¼?C´K&?î`ÛQØ?Ÿh·XÚ'L?©ÿ'J«F?Ÿh·XÚ'LAGN4FGL J2157.8+7142c¿ï{ ò‹@*˜Þ 3çŽÀ:)öi~HÛÀ;©Â@ÐO@š6ªŒ1@;7T*?Ñs&hI•u?á©ñÖq'=@	ÂzÊÒ?ç¨"õ^¢‰?Ñàu =)¿áx+ŠÈE¿ê7\Wï«¿éò6H'iI¿í"bøóœD¿ïðà<ì™UNASNone?팢,\¡¹?À¯'œJ#?³šîœ¬þ¹?À¯'œJ#?Ö
¨
ܹ?˙OჁï?äú«ú'£x?˙OჁï?ì:'Z«-?£ÝV€òÇ?¾.Ç5*¦"?£ÝV€òÇ?ÏÈ/¨¨ïè?®d&:êF6?è
ôÕÄ?®d&:êF6?éåØtÔEñ?È®hL‰_T?Èhž,®è>?È®hL‰_T?°Må\?å×?¹3Šå\ø?íöCTNÇõ?¹3Šå\ø?á¼'âX`z?·¯&v³ÑÙ?܇°;O??·¯&v³ÑÙ?'¯Î;n4v?p‡1ʖÔP?ïµ@dž>?p‡1ʖÔP MIXED4FGL J2159.6-4620?ï&Ò:'¡¸ÀI=žÇÀ:—õL¼À<rÙ	1µ@!)n'E?úN¿ÓÀ?Ãæ[L
?²ÓF¹wÛY?ðî¸Ê·H×@5Ä:, Å?ïç3€`°¿ëõðý®—¿†4›¾¶¿ÒÓ¿ÿ4¿Ý?R[§¿×–ž<–‰DUNASNone?ïþ¿&3?0£#7ã?$»dàĐ?0£#7ã?ïõð¡W?X¢ò€œè?T½€Œ«í?X¢ò€œè?ïöE——iq?QȎáo9?StÐOûÎ=?QȎáo9?ïüBÈD?(HbÄtB??Å馶j?(HbÄtB?ïþú¨Áïh?¦@n&xh? UpEr…ð?¦@n&xh?ïÙÑD֞³?|«Õ›!?s]§>Š?|«Õ›!?ïøþ‹ƒ"×?YoZ¢Šo?LÒõJ…†?YoZ¢Šo?ï÷ìÀÞ(?Aæþµ
s"?P&~'ȍ?Aæþµ
s"AGN4FGL J2201.0-6928?åÁ;ýÁÀD†Š›ÏÔ¿À:"›¯ôOÀ<n¼‡k @ö×?–@Uن³U?ÂD²w$K?×p"[<Ò@1êÝY@t^ÅÞ)?ìh§¾öJu¿áþËí©¼'¿ßÂ^ß´[¿ãßbцoñ¿ïÿü¿ÙŸC¿ïÿà‡êUNASNone3FGL J2200.0-6930?Û%̹'Äy?ɨQÃA3?âm£6Ã?ɨQÃA3?íÏdœMµ?´)ó"qÐð?±"Û"S×?´)ó"qÐð?åZlÕb¿à?´_"‰Œè?ÕK&U:€@?´_"‰Œè?í.×ú…ö,?"˶À_Ð?¶‰@*ôgŸ?"˶À_Ð?¼ìv1æG?¶(°j?ìbq9Ü£7?¶(°j?â"
˜×Ÿ0?Ñw^B¢ß5?ÚÙêÎPÁ ?Ñw^B¢ß5?ÈáPT"¹`?³¸k•ö?éÇ«ê÷Q¨?³¸k•ö?Þ·ñƒmÌ?²ÚD6i2D?à¤>7É?²ÚD6i2DMIXED4FGL J2203.3-5009?ïý%¬Ú5ÀIWÒòäÀ:©YÿOÖØÀ<j–gµò@êNÿ—z[@Ï8à^*?ΚÞ=7˜ô?×Õ¬$5¿U@Ê%£'·Õ@¯Lejh¿Þ/]›f£M¿ãØ®¸ϧ¿êu|N/7ü¿îCˆêí¿ïý¶CôK—?è"ËáëBUNASNone1FGL J2204.3-5017?ïú¤à¹X?fj½w ?G•kÒ®?fj½w ?ïìfkÕø+?t¨‹Åà?c™"éo-?t¨‹Åà?ïYm6Ã?ŠLÅ48R?"ܲ`›?ŠLÅ48R?ïôƒ­ý‡]?FeÔ2œ¤?Vø¤îÅ"?FeÔ2œ¤?ïþ±øF^o?4yrzú–?$à{X Šˆ?4yrzú–?ï'xîÜʤ?šaq•ž…?‹aÄ>~'÷?šaq•ž…?ï'À,»J?'91^Ý?›ú d³?'91^Ý?ïDÄÔl­?À)hh¦?—geoŽ`?À)hh¦AGN4FGL J2205.0+0943?í
Ôã†^ÀA¯íúCþ]À;ÉvÖöò:À='õ`iÍ@ó{}"»@:a$Þ?Ûù©#Ð>Ç?ìlª]a/@RC;¾òï@ÞÄfKäZ?ïù"ù÷¨¿á'åÞÊm¿Îª9º`äq¿â'N
ˆ¿ð?î)‰¡ÑUNASNone?î¾óiTéx?±:²»¹?¤Éhùš‰?±:²»¹?î¼Ä×_ø¹?°|Yè—æ?¤3²‹¸Bm?°|Yè—æ?ì¨îwR®	?¤ÊYח?º¸ŒEj¸?¤ÊYח?í̔¡?ÞÆ?˜Tª[›¢¬?±›ZôI;Ô?˜Tª[›¢¬?ëñ¶Z^_ ?ÃF‡¯Ú?À9&–†ƒ?ÃF‡¯Ú?ãaØú†€?ÓF"®Ö—§?Ù<Oð
ó?ÓF"®Ö—§?èikwƒ€d?´Ç›. ûƒ?ÎZR!ñþq?´Ç›. ûƒ?ãL²Že¼{?¿ôšh˜è?Ùfšã4‡
?¿ôšh˜èAGN4FGL J2205.8-8254c?ê[ÀçÖnÀ@+L`RPÀ:·ìj÷ÆÀ;ŸÌiiP@Y7žR@Ì}´'m?È.ªb?ªË¡~•\H?àV<'gMí?ø:*¨öü¿ëÿ!HO$+?¾™‹¬Æòî¿ì¨ X6¿ãÚ«'!ü¿ïþ/ ¬ˆ_¿àò«ÿ!Þ¢UNASNone?ï鳧Ã9?i~ˆ´Øƒ÷?fLêDþöä?i~ˆ´Øƒ÷?ï¸1_ÒF?'¾ò$½R?ó¨Ù$?'¾ò$½R?îyp*£[?™­§*—Qm?¨hþ°ÅfC?™­§*—Qm?ï¦x«ž
?pu¶îš¤?†aÕ|ŝ?pu¶îš¤?TPAê?"Sr鍕?‹*ï_!b?"Sr鍕?î3(
1¹-?¸Øµ–Øҝ?¬Í1/ð*?¸Øµ–Øҝ?ìÃíözE?¦UºßS‹?¹à—ðL-Ö?¦UºßS‹?ë	 A,ßÌ?²"¶ÿўþ?ÃÛ~ûL€Ñ?²"¶ÿўþ0AGN4FGL J2207.1+2222?©
qñO‡)À:‹…ƒb°À;EL¢pñÀ<¤«ë«µ%@!/A0vëD?üãÙßö?ÌÕl®ì?®4'$D"?äfwŸ@B{pcÀ?ïùß?>¬¿à;×|S7µ¿ß:â
¿ÚG_:":½¿ØA«0šÒ¿äؼßï¿@UNASNone?ïÿ&4X]u?nÊÞK?9zó<dÿ?nÊÞK?ïíÿÝà	?fqrʾþ?bû^™S?fqrʾþ?ïøW^³Œ?Aj㷐P?N£§"ùx½?Aj㷐P?ïú}§(?, Å öº›?F	b p‡ý?, Å öº›?ïÿKç¬n€?m—6þž?ƒc.?m—6þž?ï¡ñÓ}§1?•û§Éè?‡ƒ‹&—É?•û§Éè?ï÷Ŗ͌e?^V]¶‰G?PtÑãµæ?^V]¶‰G?ïîÖ{»üà?RbÖfºe?a)"D W?RbÖfºeAGN4FGL J2208.4+6443e?ïdþûÚ<³@—Óºý—À8ꈟvRÀ:þNôYÚ@
¹Ø©Nî@ǝZï9ß?«z}þDN?Ê(dM1Œ@)'^aµ'@D¼(?ÏÝ5$Ïî¿ßi<x¬9¿ãjMT¿æ;5`4>¿ìŠþ_kö¿ïÿøsCÄ{UNASNone3FGL J2206.5+6451?т!¾ý½l?ϫǛ¬æ ?ç>ï !J?ϫǛ¬æ ?ÅÚ.ºcÐ?ÁKùčÊ??ꉴQg?ÁKùčÊ??álO«Ü4?¶ÉO†ÿLÍ?Ýñ'`¨G™?¶ÉO†ÿLÍ?×|q–¬eŠ?°‹§oÜa?äAÇ4©Í;?°‹§oÜa?c,ɘ­?œ[+J½?ï|ã–pwë?œ[+J½?–ô¦ð0¬?  !1λ,?ïHZÈV#+?  !1λ,?Âïc*>9?´»I
o?ëD9'5pr?´»I
o?•3Úџ?Ÿ7'†?ïVgOfçã?Ÿ7'†MIXED4FGL J2209.2+3710¿éu÷‹'EÀ.…yRژÀ:¸dàTÀ<D»ñ³6@êkñÕ¥@a
¿cí?Ƕ5?Ìt?Óóm_ÿÄò@õ*Ÿû ?ûãq#®°Ø?ïçz,ìÈ¿æàyó$÷¿ìܸÓÅ¿è]æe$G¿ïéºy
2¿èt¡B‡NUNASNone3FGL J2209.0+3652?ïAF,›?£o=Fÿ».?ý7ßÑrŠ?£o=Fÿ».?é²PE+?Æ-¸¦hú?É7â¾ëQŒ?Æ-¸¦hú?íö"\¬ºo?›Ð«ü(â?°KÝä?›Ð«ü(â?éH5艻?¨¦bô¤©®?Êß(]Ûí?¨¦bô¤©®?êvC_"ÿÆ?ÃU@tö]P?Æ&ò¬é?ÃU@tö]P?ÊäÚf#±œ?ÌàûÙi?éFÉfw™?ÌàûÙi?æýÙ$m?¶ ãÕÞá{?ÒM·ÃÑ&?¶ ãÕÞá{?śïµ/!V?©Þí¬Xr?ê™´7«?©Þí¬XrMIXED4FGL J2210.2+5919¿ïü!
@
¶ÿÛíÒÀ9r)=æë\À;íÂÚ@l—ù±\Y@´¯Ÿ•\?Îpc?jy?Ï陌- @Ž_f—äŽ@·ètH&_¿ééÞöšüp?È#Á{4ÿ'¿å×<Èk.¿ëÚß_ ¡á¿äʝþ-B¿ïþé6ßUNASNone3FGL J2210.1+5925?ï—IV­ƒ?žŸéšX?Š=-­Ä;1?žŸéšX?ê»0‹Ê4R?']JˆåA?Å=Ð×.·?']JˆåA?íCxRw??¤'ýT:P?µä=kk??¤'ýT:P?ìSG'æ¢? ¸]qMµ?½eÃhÊï¨? ¸]qMµ?ëYáü<"ž?À¬Þ½1›¦?˜x
í‡?À¬Þ½1›¦?Òþ#Žqê ?ÒlDzc?æ€î8Ç
°?ÒlDzc?⟉	uìä?¸ùbXNf?ÚÀíí&9?¸ùbXNf?Í02íèü-?·È;k܊?è³óD…Àõ?·È;k܊MIXED4FGL J2210.2+1624?äî¾ßχÀ?€6†¤ÊOÀ:ë 8ÛêÀ<e¶ü@ôMãÕ@Ñ=?%¯½?ÍFž6€?"i:£ŒY?À+Ëö8+@0w±èDø?êð
¿0W¿ìÿÒ]°¿Þ^úâ3ç8¿ç›Þ¸‡›j¿Ú«žê;r¿ïý©^2»>UNASNone?ïû—
@?;Mä Õ›Á?A£Èƒ½5?;Mä Õ›Á?ïêÁ°A¯U?hÒãÞ%€"?e>OÂp2"?hÒãÞ%€"?ï×YÞm´?tŽ•Ìõë?tS²xX?tŽ•Ìõë?ï÷KZ5Dt?6ZÒ-A…ÿ?QiLj–í?6ZÒ-A…ÿ?ïöëK_qL?NÑS%Ù\	?R)ir—Ç'?NÑS%Ù\	?ï™o`Ç&V?'UË]?‰¤'Ã疕?'UË]?ï±fÕÄ~?…õ;?ƒ¦wþ0Hz?…õ;?ïÕfG÷TO?d¾¤¶CK—?uLÜ"¨'?d¾¤¶CK—AGN4FGL J2211.9-2924?çb_VãÎÀK|]¥qÀ;X°ô)2À<Ìõ¢®ì@ºò°Œ$?û'SÚr§½?Öã܉Ù2?É_ÃõbÃ?ò¹K{(•J@{ëöD?ïÿ|'1ž?¤Gò\ÿ4~¿è?k*M±¿»	<¿¤¿ä<~`ƒ#¿ä§f pbêUNASNone?ïñüöF~ü?'«M4áë	?\¯{(x?'«M4áë	?ïìžFQž?oc²khù?ca¹¼ mŽ?oc²khù??á{?ˆõÙR'n\?‰Ð°˜(?ˆõÙR'n\?ïöiíj¸A?<›"îÍ?S,%SÊÎ?<›"îÍ?ïý/¥"þw?9wP_ðވ?6'×>èÑß?9wP_ðވ?ï˜- n—Z?''¢QM\?‰ô—õˆ5w?''¢QM\?ï"	
)Ø?ŽOy-÷Ç?Žý¼µ¦¶%?ŽOy-÷Ç?ïåkWøöˆ?^ì<ù¸l³?j"§ä­`˜?^ì<ù¸l³AGN4FGL J2212.4+0708?îG»Æ??ÀC=lß&k¥À9ù틉5žÀ<'÷‹½8@A•Ò¯`@Äô@¯¹?¿: 8ˆ÷?àÔ=ÿêÜW@ñüLY@DeÀN9I¿é›¸øÚqÑ?Å¢7"/ü¿Þ€Ç%CŽ¿å˜Ôýó¶F¿îŠ4¡È<D¿ïóðÈT˜UNASNone3FGL J2212.5+0703?¡æ~ù«I?¬Í¡ä¥?îá˜W'?¬Í¡ä¥?˔
ˆ‰?®Xççt2?éý]ýûÞ?®Xççt2?ÆÐó«'q?®ìœV$‰S?êËä?®ìœV$‰S?Ð$	H—ã%?°ºƒoYÖÀ?çíû[´n?°ºƒoYÖÀ?c8 EàRô?d¡=֐?ïìÇ_ê:5?d¡=֐?¢L¨V:k?¢h‰½i¿?îÛ5z'Ÿy?¢h‰½i¿?š˜¹Å•O?ßËÏn43?ï+:1îÔM?ßËÏn43?ƒ^Ÿþy¡?sAjŠ`·=?ﳆ…žB©?sAjŠ`·=PSR4FGL J2218.5+6822¿í‡¹›}Ü@#"Âß
A1À:ôنïrêÀ<Xu²3ÄS@ È®Õ@
â?þç,yێ1?ÏhMÇ3/Ø?Ï`•ÁóªÝ?û>[ØÉ@Tdù7¿æ9€ô¿ïÕ E…EO?ïÿat¿ãsBí»¿å{:3µ¿âÚ!I%ã¿UNASNone?ïýéÓÿØ#?1¸*qhÐ?0±^ué]?1¸*qhÐ?ïíé=¬ïô?f/Ùº+—?bÂ)Ô¼e?f/Ùº+—?ïã	)õG?l"pÒài
?l~ö²NÉH?l"pÒài
?ïÞA8{éÓ?\Z¥q?pßc͹"?\Z¥q?ïþ 5™XÆ?*aSáFò‹?-ü£¯)Œ¦?*aSáFò‹?ï•ãÌ:"2?–1ÒóÈÞ,?Š‡àIgŽ?–1ÒóÈÞ,?ïËÔÂd"þ?\;I=ì?zž½çÌî?\;I=ì?ïŸvl?|
ŸÃYÒs?ˆ"x°êË?|
ŸÃYÒsAGN4FGL J2218.8+4736¿è¤–óՂÜÀ¬'ªÀ:ã5ï¦À<À®	"&¹@©¿©MÂ?ÿDâ–?Ë0‹£Œ·‰?ãæÀhæH@ªèžºjÊ?ÿ½Qӟ¿ëø˞#—	?ï͚R&=¿Óý‰ƒ!7¿âȅufοïUŠáoò?¦M®ß{ûúUNASNone?ã1ØSŸ?Èî+lPœ?ÙϜO×XÂ?Èî+lPœ?á	í>²B?ÌÒÍU;y[?Ýõì%'›{?ÌÒÍU;y[?áj<°ú"4?µ¶¼´v ¸?Ý+†ž»—?µ¶¼´v ¸?åL‹O?ªÅB5vÝÂ?Õfé`"ÌÖ?ªÅB5vÝÂ?Ñò¢
gž?ÈëXÉ4?ç·®úÌ1?ÈëXÉ4?»¬	ˆ¿×œ?ÁZ«@Ϻ?ìŠ~Îè
?ÁZ«@Ϻ?¹aÜ3G*6?¦#Ä婐Ó?ìÓÄyRbŠ?¦#Ä婐Ó?Â0vª×.¦?©x)ß?ësâUJ4W?©x)ßMIXED4FGL J2219.4+3229?́—íá´À4F¸Ø#B$À;r:âTÀ<ªXÆj²ü@!i´6Rø?üÊáö)½i?ҚÂïH£?¿Šk©F_á?òs§Ös?@å"…à¿ïþtDuzÖ?ïõ´bÕ¤?Ý:ÌÏ€¿äTíB83ﻥ°Bi¾¿Ùœ	€²BUNASNone?ïÿ\Úª
¹?èö ¨¶?d¯Éý·½?èö ¨¶?ï횎"4?gÔV¹2+Å?beéc½[ï?gÔV¹2+Å?ïî"òºêo?\õ¨M8…i?a{
]ÒÁH?\õ¨M8…i?ïù»"³ç¬?7ºÙq¬-Ü?Ithњ?7ºÙq¬-Ü?ïþx!éx™?)2ŽA$¤+?(}Þ¥ª?)2ŽA$¤+?ï«Z¾´Ó~?RCÔ¼?…)PV:¼m?RCÔ¼?ïßêYá®í?uM™P?p
Ó8MV?uM™P?ïëjª¡\d?\gtÅX?d•U.‰?\gtÅXAGN4FGL J2219.7-6837?Ô&)ØÀEqûçl‹DÀ:ãsê³g¡À=§"ïQ@¶`Ï£–É?øvd«{Cm?ʶI'¼1Ÿ?åU2âUu'@	­Ý|é?ûÚý‡TȄ?Öž 'ðÙ¿ÔÇå</[7¿´•M.±ï¿àµFÓù縿ëљ_â隿ïo)­¯PUNASNone3FGL J2220.6-6833?äpòªh/%?Ìوè‡Æ?׫/¡·?Ìوè‡Æ?êOOt?ÄN!¨àù?ÆëŽÂ-À?ÄN!¨àù?àák©¶.?³Â[Ïß{Ñ?Þ=(¬"é¤?³Â[Ïß{Ñ?éÉ·w-½?ªc½ç+	?ËüÙ"#I?ªc½ç+	?е]U¬Á?Ãú"Šòóä?çþ¥QU) ?Ãú"Šòóä?Ù'­02?ÒV¤kH'?ãt6©gög?ÒV¤kH'?Ѝ¾]âøø?±wºYE ?ç¹ Ñƒ"?±wºYE ?ØÖ¡…Sïõ?»»ÚÐàF–?㔯=V?»»ÚÐàF–MIXED4FGL J2220.8+6319?ï´¨+‹Q¶@ßßã*dÀ9Қl'qÀ;%/<-®@` §@~Ú4"\?¿7¢®–*ú?Öík¾?j@»øáþ9?ÿS¢F'^ã?Ó¬îàóË>¿×>l'	Z¿èDîs¿é†ýY¿í'T~1‰:¿ïÿ΁ز´UNASNone3FGL J2221.7+6318?¢
1g*?¬tÁ•X?îß,?¬tÁ•X?Á	¬yùžÆ?½u»i´4â?뽔ၘO?½u»i´4â?Ø®ú2¥]Œ?³³E÷ô§?㨂æ­Q:?³³E÷ô§?¿Fí$[)?žƒ¨Ú¯‹?ì"[tšÝ?žƒ¨Ú¯‹?—"Kt_²Ê?¢¹épF?ïCݤOCú?¢¹épF?''ÎË´Ý?›nv…aa?ïoëq—`É?›nv…aa?Â'`¨H"?°Q¬?­»?ëv'ÛÕíø?°Q¬?­»?aïÂôå¥?M˜¸ŸA½?ïîé .c?M˜¸ŸA½PSR4FGL J2222.1-3907¿àêJê	¶ÀLfѝìåqÀ;»HCe°^À='ÌÍ£Œ@ /ƒ)j²@
­¾Ìf?ϳŔÊ'?"½l˜À¼Ú?É B€-6ð?ó—8¦d®*¿îñù@É?騣ÂèG}¿ê^°Å/Iš¿Ð¨n^,†¿ÑÌ1|#çç¿ïýëóفUNASNone?íØc¯Z~¯?ÌjeP´ð?±<ℾ?ÌjeP´ð?ï²ú4¨Âñ?›mŠb"à?ƒAràv
«?›mŠb"à?î)"83x(?¡‹©:þ,?­g¼}¤d‡?¡‹©:þ,?ïí<ûL"?QKñnbvQ?bÃו$­?QKñnbvQ?ïÕé
†¦?…ÖyË}TZ?u?*h¾?…ÖyË}TZ?î2¦¶Àá?½š!‹¸Qã?¬ÕŸ<ú?½š!‹¸Qã?îⲉ¢?¥¤ …\zô?¯þ±Ó—ã?¥¤ …\zô?ï|yávÈ?†:–fϼ?pÃÊ`/?†:–fϼAGN4FGL J2222.9+1507¿ê±ê즦ÀA<fÙ×À;]`—Ì:À<¬ŠLõ|@éd'%ÜÞ?ÿ'ˆ˜ÀUÆ?ßuaù±?µVóרî?Úèpa'ëO?ÿßY´Ò/7¿ë°ýñ‡í¿å'¯Šœ¦"¿ç·ëÿ—û4¿Åóµ™ÕT¿å³ÿvmE¿Õ—®\õ#ƒUNASNone?ïþ‰%‹³[?1t^Åû>??'m¦kK*?1t^Åû>??ïé͵¼ ?k¨ÊS?fù27Ý?k¨ÊS?ïðBÅ"?gù´"%?_{ô–¸O?gù´"%?ïùYˆ»©?3ͽg…?J™Ý'¿êŸ?3ͽg…?ïÿ@8Ę?ÑTóÈ»?øß;×.¨?ÑTóÈ»?°$J?'HaxûE?Œ"«Ì§?'HaxûE?ïï6¹Gg?qÜVƒ}Ï?`ÉFãšÀÊ?qÜVƒ}Ï?ïÖucçÜ?hã²óÙë<?tÅ}Â]f?hã²óÙë<AGN4FGL J2223.0+2704?ÃEv™[ӈÀ9£œQÚ¾À;0<{±QFÀ<‰SŒo¬@=:ªËÆ?ü««u+%?àQ>¡{eQ?Û…;=ð?û»'øme@¦NTvÏÀ?ïñªÒ§a¿àç}mi¿à͒?2D÷¿Ýi'z™#R¿ïÿüoQÇs?îû¬ž¯7UNASNone?ïûJu]éÚ?H™Æ2àJ?BÖ+zÉÓÞ?H™Æ2àJ?ïì˜ø'€ÿ?f²«h@³?cg2e¹0?f²«h@³?ï)/Þ¬k?Ž"Dϑ?šÚ
ß³?Ž"Dϑ?ïó¡€ve–?CÆ©?íÛ?X¼ÿƒèF?CÆ©?íÛ?ïûK	‹Œ?LL Ð[?BÓÙÓ1Y?LL Ð[?ï£|#ä?"T(WTS(?‡ ÿð^Îø?"T(WTS(?îñÇDÄød?–zua[.? ã‹¯dö¾?–zua[.?ïÔãZ
–?g°ËD "6?uŽRûdä«?g°ËD "6AGN4FGL J2225.8-0804?¤âÕ¦ÀITÃóà7
À:Õô_¸Í<À<xÀ²¤-@ z@Ï~?ýæp­E£?ÈëæB"¥?À›Æ…
ƒ?ö×#gäè@ö/ýV'¿ïÿ¤Dî?ïËŽz\¿ÚÞ߉gó.¿Ý6çˆ9õſَÁ#vQÁ¿ãU§11Ñ3UNASNone?ïþX:À?!Ïðwù–?*~Ý-²e?!Ïðwù–?ïèBG‰g®?o¡©–8|x?g½¸}w‰€?o¡©–8|x?ïð‡jJª&?Yˆu"dî?^ñ+\íDP?Yˆu"dî?ïð¦!M"Ã?E…<'V®?^³½""*?E…<'V®?ï÷N¾T?U¢*î^5?QbƒGe¡È?U¢*î^5?ï(³—5€?'=âKªœx?‹õÓ¢;ú?'=âKªœx?ïée}÷ìO?qòW=Ü	?fšÎZAC?qòW=Ü	?ï½öŸræ@?r3ó°8ÿ?€'X#ó?r3ó°8ÿAGN4FGL J2227.1+6455¿€ƒ†]€Òa@Õw–9'ÉÀ9ÔyìU(QÀ;FT$D'ç@ß}­Õx@	Zìeˆ?ã…Üî'ÿú?ՀW¾­Ð2@'}ke©¨@¥ºIg}¿ëÓ>€ï)?ïô ~$É
¿é'‡ÂÀð¿ì(ԟÿå(¿Ô$ÀS퓿磢AˆáUNASNone?ïi­Þu×?«QºøWø·?'ÊD*~
4?«QºøWø·?ìQ£[Vú?ÀìœÁ`??½rç5%H0?ÀìœÁ`??ìo¿ 5â\?¨q|S"zì?¼'þPí?¨q|S"zì?íŸo
òÙ?¡Aª,Tjè?³‡©K 6?¡Aª,Tjè?å$R(ô?Ó/¥t™/?Õ·[ÿã®?Ó/¥t™/?Üææl8Àï?Ö_0»ùY·?ጌÉ㟈?Ö_0»ùY·?ãªËNX¹¼?½K\p€$?تicNŒ‰?½K\p€$?Ðè'´v?ÃýN%c"?ç‹ÿl~¥Å?ÃýN%c"MIXED4FGL J2229.2+6421c?¸"<»Üµ@v2~ØM4À9÷Å&p­À;k3—Ý÷@#Ü­ ¡@Ÿ!Í°"?Í,õ×]?¸'à™³Dæ?ñ`Ñ·Xâ@FŒªó´?ïÉ©—=žÇ¿æbڻοë$Äpù¿Ûg則¿ë¨ø5u¿Ý¨;¾/áUNASNone?ïù2ÍÌjì?JYxøƒÎ?K4ÈzÄ7?JYxøƒÎ?ïãÓMV?oËsÞÎ?løî%ÓrZ?oËsÞÎ?ï"e£Ùõ?‹qøÎu?Žæ—ÑoÔ?‹qøÎu?ïÁðÃL?aE‡¾Ž½;?w¯‡þ£?aE‡¾Ž½;?ïÈ´Q€Ñ!?'4cx?{¥×Tå€?'4cx?ï ¬ Àûï?£€9¿oÐ?›ê{â¹?£€9¿oÐ?î!ìIð"?£ò¸Bù³?­á;s€Ü?£ò¸Bù³?íÑ&"'™u?š¼‹/JOÂ?±vËdµÕ?š¼‹/JO AGN4FGL J2233.3+6530c¿èš+ì(Bû@yw JÃÀ9¸3¡<]À;U¡ZX;*@¹–J@6>Ðö'9?Ä×ñXP?Òc^߉gó@Gª%Øם@ÒÒË>'¿ÕÖA?»VÙ¿áÞó?þѿ檀¥+ô¿ç9¾'‡.]¿ïÿþªJl¿ïÖ¯¤ÚUNASNone?è¥IšË]?Æ¿ç>Ç?ÍjٔӮ‹?Æ¿ç>Ç?âµF¸˜"¾?Ë~k§³?ڕrŽÎö"?Ë~k§³?ë7Iÿd?§×
z^bX?Ãï—"Øq?§×
z^bX?è‹AK=¯Ó?¥¬d$&VÕ?ÍÒúÓ	@µ?¥¬d$&VÕ?ØšZ£~d?Фv±&?ãõ²Ò®@Î?Фv±&?·Bû{¼?ÀÀ•ýóË?í­àgM0?ÀÀ•ýóË?Ò¤Ýɹ
è?³âû"WâÊ?歑#zŒ?³âû"WâÊ?¾.!ïq›?¤s҉Êû"?ì:;ÂÌ ?¤s҉Êû"$MIXED4FGL J2234.2-4156¿àU¯Jþ"ÀM2ÃC·õÀ:¡HËJìÀ<ªº€™îS@etùÒ?þ&~3⅜?ÁÛY£ï?¿5£ÐÕ#?ý'ßäÅù@
šZ±ý=®?ïÄÞ˜¯¿ÙÖä¾0&ä¿ÝPd[õP¿Ý_Z©™Â¿ã7PcÅ¢6¿ä©N½þ'äUNASNone?ïþØ²´?-lÐÂ^ŒŽ?'ât—+™'?-lÐÂ^ŒŽ?ïöEI5S?X°
¢øŒr?Sumcßd0?X°
¢øŒr?ïê¬ègN?u˜u+JŠ?eS»Cɕ?u˜u+JŠ?ïþv‡4«ó?Ÿ)5n"?(—‹ ¢ ?Ÿ)5n"?ïþ¯
D& ?$ïü…f^N?%WzÞÊÛ?$ïü…f^N?ïÚµÕܸJ?|BEíEK?r¥'¡[?|BEíEK?ï삃Â0«?qCìwº²?c}|2Д²?qCìwº²?ïü­¿ã§§?+Ëoúî¯?:'ÿEX/Î?+Ëoúî¯AGN4FGL J2234.8-2610¿¾eÙä"sÀMǝØ'tÀ;~õÒ-_À<óPúÄW@ '®K½@Jv¾£>^?ËJ´C¾ñ˜?'úu7˯}?ÇnÕö— ˜@.$kSŽ¿ÍïßáÒmv¿à1ǂàð¿Â°…ƒâù	¿â$`JmŒ¿ïþÛ"31?ïø'K‰ÁUNASNone?ïõæƺ?QµÖ.'9?TyÒá-;Ö?QµÖ.'9?ïîËâìôµ?k÷ ºâøß?a4ë'?k÷ ºâøß?ïB	‰Zv?ŽWéÊ)F…?—¾ÎÙØ©?ŽWéÊ)F…?ïú)Ît[‹?6.Ôlµn?GXÅ@†}y?6.Ôlµn?ïõP€[Ë?Uns7ɇ«?U_@?©Å?Uns7ɇ«?ï§ø³õ)Q?‹LYá"
T?†Ó%G³?‹LYá"
T?ïbù‹‹}¼?ùÁÃ'™?" Î‹ ¬‰?ùÁÃ'™?ïèÕQ*¿ò?]óËÝm<Ç?g*®ÿÛ5§?]óËÝm<ÇAGN4FGL J2236.9+1839¿àµ²üAÀ@æ$Ý/ À;+k¾"üÀ<²³	­'ì@ ¦·ÙÁf?ú»iGÂ6q?ÛGaS.Ô?Շ­¾êŒ?÷æê…Dwÿ@'Q8×·â¿ìÛ;$™<}¿ÔW­Ñ_ſ堕 ãû=¿Ö3ÍA¼¸Ø¿ÝÜæ ]ƒ¿ï÷mõ¦àªUNASNone?ïúÏâßf`?:JnhÕ4?DÀtÙÂø?:JnhÕ4?ïæF{9‡5?kÝx6¦û?i¹"¾9ºÍ?kÝx6¦û?カMÁê?yì¼Í~O?€'lÄÆcg?yì¼Í~O?ïðöÍÌç?FøÔvUˆh?^e[ò°?FøÔvUˆh?ïù¬Éø6?Jf#H'ù?IL؁5¯'?Jf#H'ù?ï†Ã"K{Ì?"þEíTiª?ŽO7zß|ú?"þEíTiª?ï¾àMæ›^?'­'MqVë?€G셩<š?'­'MqVë?ﯬOï?yru"Sœ?"ø8&?yru"SœAGN4FGL J2237.2-6726?ïÜXãhgÀFq€AÀ;¼Ì¤‰À<Ó+—]7@ 3M«?ÿŸMR™*?ÏäÄeJ2?¹ü*9?Á")Ǥš@÷Ÿúêü?å).—ÂÿÄ¿âæŽà3·¿âoÒá8ꂿÜ)•»»¿Ú½ÒÉfÿ¿êKWÇýUNASNone?ïÿeq°Ì?	âÙ½iL
?QÌÆRš?	âÙ½iL
?ï÷:S?V	È蘄?QÿÙЧ‰?V	È蘄?ïõñèÔÙû?jl'¶†jå?T.‡Y,?jl'¶†jå?ïþüú‰jð?üå´<Î? 0V®fF?üå´<Î?ïÿª2v¨\?V¾GRÓ?sV ¨¤ú?V¾GRÓ?ïܔ'ꪮ?{@°‡çQs?qµìÛ4ç?{@°‡çQs?ïùÉp³±?b%Uhø'?HÚ<W…d?b%Uhø'?ïýjå­;?&É¿©»éð?4¯gÖÌd3?&É¿©»éðAGN4FGL J2237.6-5126?ìtMÀ
ˆÀK"DAxpTÀ:ÏfhæÀ<bÜ¢c@kíR@…c¯˜?Ó4Ú–Ž¢?ÙPê°£?ø
e~ßÙð@äÀ»!ª?íÁI̽¿èC}ÎaøC¿ï#¤FÞâ¿àhŸ[zz¿äk¼|±¿ï³¹€iÇÅUNASNone?ïûÏì^Yõ?XP2qÜ?@ÀOHÅ?XP2qÜ?ïð5æ§ûm?ng¢bØGÃ?_"2eѕ²?ng¢bØGÃ?ï-(™ÉŒž?"8P¢†‡?šZìÅžH?"8P¢†‡?ïúmÏÜæ?4¤]k|$€?FHÂä5çÓ?4¤]k|$€?ïý&×ã´Î?HwŽþãŸ4?6ÉAWÿ_°?HwŽþãŸ4?ïÈÏã?†ì`¶¿?{˜yن,?†ì`¶¿?ï 9¹è¢?"_òêÿÎé?›øÈÄ£Š>?"_òêÿÎé?ï¿Smmõ/?u®R/m?€+$«	öO?u®R/mAGN4FGL J2240.3-5241¿Æb5m9ÀK[I@»±òÀ9Ç]b±¦À;',kûÒ@ Ã-nÎõ@4M:'£?³ÈJ±ÿì࿦nJáO»ª?õöÁ]-Á@eÎà"j
?áh æ)•%¿ëšJ~©SK?›"*zä¿åYa/ÅÀi¿àÖÔBaúF¿à¡ýì)‰fUNASNone?ïûRTÇ¿?p†=…íKe?CÒ¶å)Q?p†=…íKe?ïõ,'ÃO?XÑßvÁª?U§õ?Æ3=?XÑßvÁª?ïÙ|ð/lC?{ƓX%Ã?sA‡õXbg?{ƓX%Ã?ïö'ãA$Û?>ÅÅÈ O?Rú9Nûš¦?>ÅÅÈ O?ïõö4WÔ?P¸_¦…o©?T—×¥??P¸_¦…o©?ï؉b®º?|ëU¬5yÉ?s»N½UË	?|ëU¬5yÉ?ï¼!iS×?†2,{r¸?€÷¥¿Êâ8?†2,{r¸?ïÒPÉw`?k•÷/Q)?vכ^Ha?k•÷/Q)AGN4FGL J2241.2+4303?¹&ú¬{À+dî
öÀ;µ^>JÀ<Ô6>@lf EoÌ@øBf¬ÝC?Õ5¯D%ɾ?ïÿÜ>Y×ã@R%1ðÃ?æ -Š&ßé¿êŒëÖ}O·?k`ñ²_¿áæ͓œ*¿ït¸¤ Ü¿ïñÓíR~R?á 1ί%UNASNone?é=§Ú"Θ?Íì8~Kµ?Ë	`•°ÅŸ?Íì8~Kµ?Ìåp<~
?ÇÇ@AŸÃ»?èÆ£ðà}Y?ÇÇ@AŸÃ»?æt3ƒ?±'dÒqå?ÓÙ˜øßÐ?±'dÒqå?²ÔÚ4ÚÌA?œ\¦+õ½Œ?í¥d¹› 8?œ\¦+õ½Œ?å¾îf¿@Œ?҂zb`Œ!?Ԃ#2~è?҂zb`Œ!?§";e®5?®ôÍ7ú?Iò½L?®ôÍ7ú?Ó«Æ«m?µ!"X}A5?æs*~ªJ?µ!"X}A5?avöÖ²f?RpQ-)?ïî‰	o¢?RpQ-)MIXED4FGL J2241.4-8327?æÀôž;ُÀ@J^	}À:°Ù(û¡ÌÀ<…Ål†;@ýTÔî"?ÿ‡7|n¨?Êd_:£?ÛÍó}抹@Ê%ïúÏ@n½:2«Ï¿ëY@¹À¿Åù'¾8ß¿ÝÔ>{eÑì¿Þ²	Ò癿îåvå¿ï裝SqUNASNone3FGL J2237.5-8326?ï
ºßÿq?¢*·¹•7Š?žH¤Qè?¢*·¹•7Š?ïÊðä%¦O?{>ñ6Ç?z‡üûT?{>ñ6Ç?ëÃתïå?¨»/\ã%—?Àð¡Tñ@l?¨»/\ã%—?ïo\vÎhƒ?sÏ+tiˆ¬?'q'꽔?sÏ+tiˆ¬?ì°/Cu²?µÌb_<ð?¹ê~…äRr?µÌb_<ð?îþáHÒ#?§?wƆ? ñé»Î?§?wƆ?ÚbËvý?½ŽûG{P?âΚsDu?½ŽûG{P?ëø§Bht!?¨d£øÖª?Àbö^/z?¨d£øÖªMIXED4FGL J2245.8-4148¿ïù⡗·9ÀN=þ!ÙnœÀ;"E	Œ³À<ïð‹î¶,@"Y‡°¸ð?þ'Ù--_µ?ÓJ"ä(3%?Ï8ùÜ$ƒ˜?÷çESÇ'q@_Î$1?Ò¬cû¿äì¶wò¿¾'¡T£ñ¿å}Ä@âl¿á°'¿ŠÄë¿ïøž;ê½UNASNone?ïü7{}‹?6û¨'eÁ£??fBñP#8?6û¨'eÁ£?ïîýPùØ?feýW¨Œ?a¯8cˆ?feýW¨Œ?ï«=ws˜Ã?*5Êf=?…0¢ëÃf?*5Êf=?ïñþ@üä1?B;­G6?\~¶þí?B;­G6?ïüaÀÂÛæ?@X!Ò´?<ñûÄ8?@X!Ò´?ïÇr*ú´?…†îÀ>S`?|FëoÁÿ?…†îÀ>S`?–6t?‰µ'
×?U»è0Òò?‰µ'
×?ïÁÂUO"?pwc{uÃ?8É©Š³?pwc{uÃAGN4FGL J2247.7-5857?±G™­Ì¾ÀIÔÖõD»À:Ñ×ÙôÓÀ<&0ì1@£Ð3ç¹@¶½2%?½5 á6'7¿¯©¬â Æõ?ñ7jК¸@"'[d±?ïüL·h·y¿èMW¡§…¿éHÆÆ"¿àMÉåX4¿éóaáòN¿ïÿ-½R†`UNASNone?ïÖhC$0Ñ?¬º&`t±n?tËÞXšÏ?¬º&`t±n?ïòH™ʽ?`C½Þ·Ô?[nÎ2á%`?`C½Þ·Ô?ïě³OME?¬æG.'/?}²&o¶µI?¬æG.'/?ïø8?4üGHã:ê?O·±
>Fn?4üGHã:ê?ïÕÐ0{ë*?wÍç"ê2à?uç´Kúê?wÍç"ê2à?ïÏÃ(օU?fK6}Ì$?xk|%È?fK6}Ì$?ï™òŽ
°~?‰/Èàþä?‰ƒ\Áìk?‰/Èàþä?ïÅÁbOD?l')}e{?}wMx…Ú?l')}e{AGN4FGL J2249.4+6222¿émœ µÎ@C±Ã\
ÃÀ9±úã`	À;ü}"€U@;ڌ(õ@¬{­?ÓÈD½IL$?ÇÉD6¶Ë?þzŽÜ§5d?á>ÚJ± –?ï­Ê¾­	¿Ü3Յ2à¿ëÝü›Çq¿æT7ûr¿ì©c`Íu>¿ïöQ*"ÿUNASNone?îoçC×?²A.r©÷¨?©‹Ñr‹?²A.r©÷¨?×'ïo†m?ÍÛ¾wt€°?älH<Éy?ÍÛ¾wt€°?ì.åˆÛ[[?¦AŽ«Ÿ™?¾ˆÓ¹%%)?¦AŽ«Ÿ™?ÔaÚù¾Ðé?² (øôR`?åσ —‹?² (øôR`?ç6;ß»M/?Ë©7köÒ?ѓˆ@‰e¢?Ë©7köÒ?¨Í¦ïÿ?¶ÊÜë½x¨?îs%'@?¶ÊÜë½x¨?âCE¯·"*?»ø%¢ô-±?Ûyt Ù­?»ø%¢ô-±?‰õú÷
@©?w°r
5‹?ï˜(ßÎ?w°r
5‹MIXED4FGL J2250.5+3305?ʬ¬h~DÀ7H`RP/À:<GËp¬;À<cþcGÍõ@cá4¸ÄW@ϑE7A¶?ÂBˁž%E?ãóÞ>d>Ä@f<ù…'@çâû{9?ÙZ…<ji€¿'Š;¾Ù*d¿âÖV¹J9¿ë²'LÃýñ¿ïÿd™ÝŒ8¿ÞBÛ\\¢BUNASNone3FGL J2250.6+3308?Áp1@iÓ?ކ'1ɯ?ë½ãó¯å‹?ކ'1ɯ?Ï`FfÁ«?ÄIÂÙP`7?è'îfO•??ÄIÂÙP`7?Ô¹eeÏ+'?²dB=ÊãT?å£MMj8?²dB=ÊãT?Òàؼ'?®ð¯JÈà‹?揓÷¡À7?®ð¯JÈà‹?Ÿ£i"±ˆ¬?¸5­Z?ïä´+ê?¸5­Z?©í†ØV*Ê?°Æa{Tú?îa''–3?°Æa{Tú?µqЁs?£yšªœß?íQÅü4T­?£yšªœß?'wÕLî³6?}
Xc‡z?ïtAUŠËö?}
Xc‡zPSR4FGL J2250.6+5809?èé/ÑKY¿ðûx–ê'°À:§¢>ƒÉNÀ<	ɓ\i@!'8úóPÅ?õM
À¿?ß}~á‡o?ÝÏ`cò@I][û©Y?óüûhÁŠy?íÝ®ˆ*Ü¿ïù¦êºô]?îVÃ[4=¿Ü«›úœê¿Û1s?'½¿ïã¡ìõ6UNASNone?ïÖOS5˜N?‰ìiQ%­&?tØVbt(Æ?‰ìiQ%­&?îÉý=i(I?²zë²lم?£`,%ýßw?²zë²lم?î±,í7À%?˜k%Æ°-?¤í1(8z½?˜k%Æ°-?ìè"6þïµ? CÊXs÷ƒ?¸»fG,›\? CÊXs÷ƒ?ïÐÑgÍU?|…ez³å?wðVh){?|…ez³å?éÛ%2r?Ðeäq•U?Ëē‹k67?Ðeäq•U?íbnʎ8?§?5ê°~?´ì‰«ýÙ¼?§?5ê°~?éY1R;Û?¹\q=VŽ?ʛ:·°•?¹\q=VŽAGN4FGL J2255.4-3252?íõ¹>X3ÀP"ÊÕ{ÈÀ:ÎCr‰ŠÀ<¤é½ž[ @ÙIŠ8@¡ƒræ§?ÐYkáÐj?ЂƒÓ^·E?þV'Tà@ÙE¡Iç*¿ãÅâB)ñ¿Î	{(ë1¿â­×>?׿æì¶!9¶…¿ê`üßåy¿ïÌvÀü‰ÿUNASNone?ïð•æG%?bzÚÎòq?^Õø8ñ8?bzÚÎòq?ïâÞž -?io6w–?mp!gRå?io6w–?ïˆ"áÆP?ƒ%°¥ç3?þš¹Ïûô?ƒ%°¥ç3?ïß—ºW?V	CFåæ?p{´ ÄsÊ?V	CFåæ?ïÁþ"bÞû? k¿È€­?îß¾Žh? k¿È€­?ïi@¦ÁÓÓ?›ªê%­vŒ?'×ë&
·¢?›ªê%­vŒ?îMLf,|,?÷™¤ãA?«+9 §Ù7?÷™¤ãA?ïfQ²ò}ƒ?'f
'?"5ɜˆå¬?'f
'AGN4FGL J2256.5+6212c¿ïÿ2|V@ "S.{>À9r« ªšÀ:íև`±ñ@R°ŽES@Äg£}?ÐD~Ÿ˜6B?Þ¸AíHm@[輜$?ñÌGVUÍ¿æmE}¸'ƒ¿«iü"0·ê¿æÔS©Ë@¿íüŠ_iòã¿é!	?nÕÌ?Åáœ}#Â'UNASNone2FGL J2257.5+6222c?éf螠¦?ÌLÜ¿*š*?Êgø]…}i?ÌLÜ¿*š*?ЅÈ`à?ÈQK÷û#Í?ç½7ò›Ï?ÈQK÷û#Í?çëAP£,?±¼øîc¬j?Ð)}_Ú¹¨?±¼øîc¬j?Ù=vÇ2j?´ôcó")©?ãaDóœfË?´ôcó")©?âOÒ§a•?Ï'¥W,?Û`[ȱ<×?Ï'¥W,?˜Ñ}†t–?¦k\O¤<'?ï9tçØ0?¦k\O¤<'?Õhu›sË?µØ0ykJ?å|ËÅ2F?µØ0ykJ?"Ê/p$?xŽZ˜Ÿ@?ï¬×ÇQ¸¯?xŽZ˜Ÿ@(MIXED4FGL J2303.9+5554?ÃðèC
­ÀàÒ=OèÀ:Åc®ünÀ<^UªV€@!¸_õ‰Ÿ?üŠ"C"?ÈÁêAÞG?Åq!Àŧ?ü£mWò/@]Ñ8Â>¿ïÿø]ˆò¿¼ÙÃUU?ïÿÎÿYg¿Í7IWâ¿þ¿éÈ}ýܺ+?ÂJÆüÔ'UNASNone3FGL J2303.7+5555?ïønCT"€?Já–NÖàï?NFòÅUµ²?Já–NÖàï?ïÔ±œ{?}9>ÔhÚÚ?u§1ò;RY?}9>ÔhÚÚ?ïµíó8z?~‹­ŠÜÏ?'"ƒ>W¹X?~‹­ŠÜÏ?ïC«G8+?"힧Á½?—Š—ú'?"힧Á½?ïÑp×>ÑÞ?uH֚ÃE©?wG"aFüõ?uH֚ÃE©?ï=I GX?£õ~å?˜VÜÎ?£õ~å?ïÕ5bH±?•åB+Ì÷?ŸeYL×±ô?•åB+Ì÷?í Ù,4D?¥¶÷Ó5?²ù6 ƒ¡=?¥¶÷Ó5AGN4FGL J2304.0+5406e?è²R=h|ÀXàkæÀ8›Òß5…À:äk篧"@#7›!Ùï?ü-SaÅ?µpb=·Æ€?Ï>;¤ò@"è‹+B?þ§mrU¿ïÿêњ'ç?ïÿ› 'V‡¿ÜÐæ7
¿ºWìPӿفà•V"¿»?#@÷ÁîUNASNone3FGL J2309.0+5428?îº#Š|?´ F…ì?¤_ÝşZD?´ F…ì?äŽ`3$"?Ò%'ˆz¯Á?×Øã?™·»?Ò%'ˆz¯Á?êóÙ¹ø½I?­+ËéU¢'?Ä0™
Û?­+ËéU¢'?æ8¹b•T?·%Oº"\>?Ó͎:ÕX?·%Oº"\>?ë½Ëb?¸áõ*0wŽ?ÁÑúwï•?¸áõ*0wŽ?ÒU]?Ó+g§ Ý?æòxUQ@:?Ó+g§ Ý?ëfWU"õ?­…š›7®Œ?òf¢©ì+?­…š›7®Œ?Â3òЀ6?µ0ž)1Ó?ësKþŸò?µ0ž)1ÓMIXED4FGL J2306.6+0940¿ïÌU&´0ÀF£sÀÁüÀ;)Î悀xÀ<†\<@øï@2gà9@‹ƒVa6?Ë'4!o¼P?¨U:Þ¼þ?Û%l 9±R?û:µÃ›Ë£?îêI¥Ò?ê©érõÁ¿égÃd™¿ãôJ?>YW¿ßJDÝ)¼<¿ïÿ!ž5_³UNASNone?ïû{&?@¿Ë³xb?BÓGÜÅ"?@¿Ë³xb?ïɄéçÃQ?‹d­·Z`#?{=Šøà‡°?‹d­·Z`#?ï̸ N?u'i<\º/?y£°t8Á?u'i<\º/?ï΋±Øq?bIAOɈ?xº'¯†?bIAOɈ?ïëÁ]i"ê?hg#@>?d>¢ØՕ.?hg#@>?îôÁMg¼Ó?¯ãæB4p? ³ë-ϵÏ?¯ãæB4p?ïzñê#Ûã?ŒÌ" u?¡Â»"ƒ?ŒÌ" u?îÓ{ŽQù?'Õº…=?¢ÈGpÓà?'Õº…=AGN4FGL J2311.6-4427?ᆲª‡AlÀOǛÜiøÂÀ;@­
ê¤NÀ<¨¯3+¦@TjX¹T @9×wJº8?Ô.]¶i‰?¼¸—
ÉÅ?éŽ_tÝÛ@¶ø¥Ò?âØ"ð½¿é³hb?_¿år¡L$œ¿ÝTŸÿå(
¿åly¥ÞKz¿ðUNASNone?ïûg÷ò&?QÍP¡÷?Ì?C²`%¶É,?QÍP¡÷?Ì?ïó¯ak?^ŸÆ
1µ?Yæ¡ÈÚø?^ŸÆ
1µ?ïáÏV¦1?sµŒËŸ5?n0©+5‹?sµŒËŸ5?ïùùËÞeQ?/E•µ5¦?HÐr 1?/E•µ5¦?ïþ\|W¿Z?/º¸ëžë?*8:|Í.?/º¸ëžë?ïÒ^ý³Â?€f7º?vñÐxç?€f7º?ï朞ª?t^u¹è?icaïtD³?t^u¹è?ïߐ‡³N]?`êÖY/ʈ?p7¼¼iÌ?`êÖY/ʈAGN4FGL J2312.4+8253?íÀv£S	p@4£ èBtÀ:œZxòZ%À<EÇwù5á@̎²µÊR@½aÀxi?Ð6>"þ?Ôq³/lÕ@ã
ù½Æ @77F¾*s?î8Çâ'@¸¿ãÚ¨ÝÚ;J¿êšÂ
¬¿íÚ)vñÎå¿ïÉ4â_Ü	¿é8âií¤UNASNone?ïÀh˜oÍî?‰õ`PM?˳Ê(Ìã?‰õ`PM?îu/‡­?«½Lì²?¨®Í	<ý}?«½Lì²?ï")º…ð?Œg«{¸@?ž-zÑFGý?Œg«{¸@?í®áÜBOu?'Ø&f(ûb?²ˆñ¥RY?'Ø&f(ûb?ïT¬Þ¬?"ì*
?žü?•jd,7\?"ì*
?žü?âH¿âX¥?Ð7»¥x?ÛÝn€;N¶?Ð7»¥x?ìEüÇøbä?©fž¶:;?½ÐÀ<èá?©fž¶:;?à]{eÀ¾?µxðå
)?ßEÏ	4~"?µxðå
)AGN4FGL J2313.4+5947¿âù	1¾$O¿è«ûèCKÀ:&†ZøtÀ;;ÌÛ…¯@ ³˜zµ¨Ä@‰~Jˆº?ƣ歰¿£$"3ÿ
?ÞÑ0ÿÒ2½?úî5r} ë?ïô`Å<µ"¿Þ• c!ãU¿è_øù{¿ç\¦>m£ò¿Ó4˜Žß#¿ë
Οµ½gUNASNone?ïöª$ðéü?Kq«5Ç»Ø?R«µÖ´'Ê?Kq«5Ç»Ø?ïÇ8È7Uœ?ˆÑ@
±û?|cœñš?ˆÑ@
±û?卵hÅ«	?ƒhn©?†ØåË%¡³?ƒhn©?ï½BSÈ?i6	ÈDî˜?€»ï{î£å?i6	ÈDî˜?ïå©ð~Ø£?c]|Wsj?jVxèLò?c]|Wsj?îP×Ñb³©?² =.ï?ªò'ìhzf?² =.ï?îÙGºÇè?˜¸k©»Ø?¢kŽÅ/h†?˜¸k©»Ø?íkH?A«?§=¨ºÆPa?´¥¾¦?§=¨ºÆPaAGN4FGL J2316.7-3144¿ÛîØ{è¿ÙÀQ;27Š°ÉÀ;=•ôÉkÀ<Â"<jêZ@èák•O]@9þ¡[.û?Æ%]‡š"•¿±=èîÁi?è¹EÁ€=}?úˆÂ>SwÌ¿ãýž%ðU¿ì´R¿Ýñ¥U¿ßgk1|¿çŠ¢OοÕð?ÃdnUNASNone?ïø$§²¿Ž?L{$C©Ñ?Om`§+'h?L{$C©Ñ?ïÖƼ3ð?‹º­†"©?tð£Eà?‹º­†"©?神Ý-º?…"Ñ‹xn§?…ûˆ´'d?…"Ñ‹xn§?ïëÎÐç[?Nñ?y?d1ü»M?Nñ?y?ïìZ9D?cÚé¥Û§?c¥ôÔzV?cÚé¥Û§?ï–Ð*i$?«±¸Q5&?ž
&'x?«±¸Q5&?ïz¾[+0?Ž†[Ðë}X?¨4"ºÅT?Ž†[Ðë}X?ïALñ @Ó?‰à¾vfÇ\?—ÖaÆÐ{±?‰à¾vfÇ\AGN4FGL J2316.8-2518?ßwH"ÕÀQ/Ë>WS¤À;j@ºˆÀ<È)ösD@8bè,¤¤@7^nÔÊ@»·Þþþx?·Ç¡á^T@r»3rH¿ïûƒ¶?ߙС½6¿Ýåâþ"P¿åÏ\>oQr¿ïþ9 ²ýï?ïøª O€ÇUNASNone?ïœæÜ~¬¿?°^wé?ˆÆHÏ&Ä:?°^wé?ïì\;íÅ?q_
y¶µ?c£2ykÓ?q_
y¶µ?íû¼ÓÍX?¤Uê×ʎ?°"fã¡Á?¤Uê×ʎ?ïü?s³V?6ّ+¸ø?>ae :ˆ?6ّ+¸ø?ïên1С\?p5Д~ÿ?e'ÎYùËO?p5Д~ÿ?ïšq¦"?' £¹ƒú?‰c–M?ì?' £¹ƒú?îÒ#g§ó¾?™"Ÿ
s€¾?¢ÝɈy?™"Ÿ
s€¾?ïå¡	8¨?hüM·!£—?j^üúæàO?hüM·!£—AGN4FGL J2317.7+2839?Ð1…Üß{À=ÜÏ|ªuŠÀ:j‰á•²À<hÇåÝ?@ [¡äì©6@'U»Gi?¹nlŒñ¿—E`dø0?àšf³"?ã@
Rí*eYK¿Õ·¼]éÀ¿ßôYĚ̿âa8ÿûοá+8'ŽºC¿ÞÇ¢@‡.³¿Ó\åGB	UNASNone?ïþëQ4?•I½LŽT?!JïC<÷?•I½LŽT?ïò=*
ž?`ºòü¬¤f?[…«õ‡u?`ºòü¬¤f?ïùR·æi_?[wA-.zÔ?Jµ!
»ß?[wA-.zÔ?ïþMaB÷2?Ê
›<s?+)í2—Õá?Ê
›<s?ïþxóJ©¶?*»["u?(pÍ%c
M?*»["u?ïć¥Áh?‡­Òd%l?}¼v™á|U?‡­Òd%l?ïûmt^?Z£ãÈZ'ô?C—þi"'þ?Z£ãÈZ'ô?ïúÅÜ¡3Ê?6!ús¡8?DèFj	ç?6!ús¡8AGN4FGL J2317.8+6140c?à›ø£.1°?é˜c8´|tÀ:݉³r‰À;"•µŠé@"»ï¯Ð¾@Gz>Š?ÉÍ$`‡;?׺šÛŽ½@
À?`h?ôΨB¿ê½˜]ƒ¿±dS爺ϿÚÈ2¾ïŸ¿éÖð¸»¿é€Å§J¿ïÿþÐñUNASNone?ìêÌxOX?»Ç±·ë?¿Ø©œ=…>?»Ç±·ë?Ú¹¶tñ™‹?Ìp©ÚÉ(—?â£$Ň3;?Ìp©ÚÉ(—?ëo!î½7ƒ?¥uÖ+ù·?ÂCxE!ò?¥uÖ+ù·?á㳎JÂ?®S8~z?Ü8™òãj|?®S8~z?ÔÝÕ©üN?Ç/e¼P…?å'+ØÀ?Ç/e¼P…?¨µW•\+?³4jŠ H?îĪO°~?³4jŠ H?Û,'ó†lc?¹¨·ªâÓ[?âiì<ÉÏ?¹¨·ªâÓ[?ªMÒG•S?"A¤
†"g?î^+"²K[?"A¤
†"g!MIXED4FGL J2318.6-3827?Éh¨Ü"ÐhÀPâpdìé£À;٘áõ²À=Jb¹3@û‹¨jAè?ÿ@[ŠjQ­?Ø9Å^?ì¢E¥%¾Ö@šð{þ~ @Ñʽf'¿ïÿå=†ô&¿ÁPɆœ;à?ïú՞­«¿Þ$#á0±ú¿ìgs¬ ›¿ïý_ÂvíUNASNone3FGL J2318.6-3829?ï߬6îîO?‡~p¾ñý:?p)äh<"â?‡~p¾ñý:?ïÞ3%‹¼?'Ÿe·È	k?pæm=ã=ç?'Ÿe·È	k?í¨5•Ûkn? dì[
ý/?²¾SP¶±? dì[
ý/?ï5å^áYC?‰@¸úBè?™CT'Ds•?‰@¸úBè?ˆ!Þ2?˜_óúpñp?‹Øð©;q?˜_óúpñp?ï²ï?':Ç?ü@¨"?ƒD0›8R?ü@¨"?ì ÀÇR[å?«?kJ²Èî?¾ùùÅm Ú?«?kJ²Èî?í'æ*RC?«èE]´†?³èΫ·7ì?«èE]´†AGN4FGL J2318.9+4151¿ÉbᒒÐcÀ1ŃùdoÀ;¿¦sœ°À<Ví½\ì@Ô¥Èüލ@™#²?ɖ÷¨Ãƒ"?®%{·?åcä
Öó—?þàUÓq+¼¿ïƒ"4?ïÅ(ÉL匿é$É®4[Q¿á@$³=¯Ž¿ëù—eâ²è?±qj{sé²UNASNone?ïù°¸?Dõ?Z§w?Kå=gäzy?Dõ?Z§w?ïáßýgZ"?xÑI¶.ß?n "&­?xÑI¶.ß?ï¦uäÍcd?€µO'G6+?†b†ÂXRó?€µO'G6+?ïҐÄïïÎ?]uC󥡶?v·÷?]uC󥡶?ïÑx|z?|—áVqNÀ?wvð6S9?|—áVqNÀ?ï=ü<¦úU?§|£ÀÒ?˜@xg±\?§|£ÀÒ?ïÔ¸ËÛX?‹
ùã'SX?ŠÑəŽ?‹
ùã'SX?îI¬bZNf?œ§…ïˆô?«e9ÜîΗ?œ§…ïˆôAGN4FGL J2320.1-2440¿ï똛S_ÀQV灃ùÀ;75c'À<°Ô8í‡@"·ç7‡@'`}Y"?Áƒúuý]8¿µ)žŸgäÁ?óÁC|V'´@mÀÐj;2?æêŒÑ4;¿èÏ_žÌ'¿æ·Î8Ø¿åù˜¨)?µáVáRÈ¿ïÿÈb±UNASNone?ïû"âÓýÌ?FKžÍ)l?A°tÕjõ˜?FKžÍ)l?ïì¯ìŸÙ'?p>\ð{]?cP2Ë¥ú?p>\ð{]?ïãĺÑïï?no&Ȧ€h?l;EEmi-?no&Ȧ€h?ïý—û^A?$•5c"?3@'½Hj‰?$•5c"?ïóÓ¡I³ ?Ypõo—‹?XX½ÁÏG?Ypõo—‹?Óýºù?pªnhK?ˆÐÊöBmâ?pªnhK?ïÃEs*?`",#F?~]xû?`",#F?ïé9¯	?bâª&&&Ó?fëÆ6Ùy?bâª&&&ÓAGN4FGL J2320.2+0707?ÜæîlÀH _ZÙjjÀ;=®¸å;À<‰é'9Y@!
/ÿL%ó?ü¸âe+Ô?ÓÔR?´J*ñpE7?ãà÷?ò=æ*þ¿ìjœ&@‡?ïw·ÒiÅ¿Û~ž¡@W¿à؆¿L[£¿ÃÏ¥ïa¿ä­rÊ!÷¢UNASNone?ïϞ ‹ó‹?±ëI:?x0¯Ð³¦Q?±ëI:?ïán¾éN?'Azâ?~/HÂçp½?'Azâ?ï˲],M]?é;]C;
?z&Ñ`êUf?é;]C;
?ïÚ$c.?`½å­7?ríÎRE‹'?`½å­7?ïûÊaô¢æ?Eä¼'S·?@Öx.%e?Eä¼'S·?îØw`'D™?°7Ø¥ÇE?¢x‰ôHp?°7Ø¥ÇE?ï»ÿ¨K¹?…¹›ë6"??'u"Â?…¹›ë6"?ïäÞ*\?'±L†q?Ãd8ü°F?'±L†qAGN4FGL J2321.9-4842¿ìvˆ&CzmÀO+Ê! áøÀ;'^±ŽÀ<™Dwÿ@ð³¿Õ˜?ÿÁ†}]"ñ?Ð
,8m.Ø?ºxîÍ?é¬ÖÝÇÆÔ@?X£Q?҇±d¼m.¿äÛ£ß¿ßfÙRí¿àìÒü'¶v¿â-«¿‹ñ¿íù> #ÌcUNASNone?ïþ§mö0Q?²hºX‡û?%‰ä½›?²hºX‡û?ïõ¡Œy—é?X9þgNì?T¼çˆ''?X9þgNì?ïòàÑÖ:Î?jJäÖ$?Z>\Ðób?jJäÖ$?ïûËòÿˆÙ?&wÈÌA
÷?@Ð5	¾š?&wÈÌA
÷?ïÿ^õ¼?I(iø?t!Á5¿?I(iø?ïÙ0Ç·ÓÛ?z#±°È§}?sgœiæ?z#±°È§}?ï÷·þDÐ%?c¬˜o8>?P^vB?c¬˜o8>?ïðG!"?Põº/Oô–?_ùq7$*i?Põº/Oô–AGN4FGL J2323.1+2040¿æ™»}oÀBÑ|o½'=À:ÚýPùØÀ<kymª'†@¯ˆc'Iê@¥ÆÁ#?ÃõB6Ü5 ¿¢ðš1o
Õ?ádðD¡?ÿº°?£Y¿è7Ïᗊ¿Ú5ÅaŸ¿ç<lݣߙ¿áʓÒ}'¿Øx\2/ýõ¿çÝu&Ê;UNASNone?ïýÀ÷Õý?"Ü%ðW[?1øGávŽ[?"Ü%ðW[?ïì«-¯y?f'¯Ù¹§§?cT҇zFé?f'¯Ù¹§§?ïé?"j…°?j˜œÒ?fÀkTᨂ?j˜œÒ?ïøvÀ´;?4ªj_Á¤·?N'è* Ÿÿ?4ªj_Á¤·?ïù2ÞØ?Bªê(˜ï?I‹5)mè?Bªê(˜ï?ï°>Ð[‰?ˆÊ–ŒòØ?ƒÿðT(-Á?ˆÊ–ŒòØ?ïÛ»Mlš?wg¿tÒi?r"}總?wg¿tÒi?ï¿2"k¡(?r>†m€Ø¡?€3ZÜئ$?r>†m€Ø¡AGN4FGL J2323.9+2519?Ä!rÇÙÚ
À@ºç¯·éÀ:Ï'`—À<‡ô9rè@¢@ÕXå?üqišÐ?àÆdÓ¿/?ڒòK—
?ü¸ŸÔF=Ò?õÑ-=û¹¿èz9¢õ¿äYÈ]ÒC.¿ãEgéel¿Úü•½Aœ¿ê¦k93þ4¿ïýwƒ–"UNASNone3FGL J2323.7+2523?ïê!Üɚ?f?=÷Â!Ù?eÞ#jŸýR?f?=÷Â!Ù?ïyT¸œœ·?šÐ]Z?Õhå1-?šÐ]Z?"¾µ¢?–#î¡Ò°ä?¤uíׄAá?–#î¡Ò°ä?îðüH9‹?"¸SÂ?˜+? ð;|WêM?"¸SÂ?˜+?ïÅW|àó˜?û»±ªŒ?}TAqI¤P?û»±ªŒ?íH"D#?¾'¸t®±6?·¿í6î?¾'¸t®±6?íÒ'ËÝæ?¡K³ÎYÝ?±nÁ¡òïÑ?¡K³ÎYÝ?ꛙҵ«.?°"0TÒ,m?ő˜µ)SG?°"0TÒ,mAGN4FGL J2323.9+6219?ïÀƒ¸?ò"cښë©À:}Ñs$ºÊÀ;™®°'k@!!|o?@«j©Ø¬?ÖÙ¶Ÿä·O?µta%߸?ßÒèûV¢ú@®6Ñ?ïýä×Û¿î/¬*•ÕÀ¿È†ëA,¿ßu§·iŽ9¿â†=œBÁ¿àÄ(ï'µUNASNone?ï÷kyu·½?X"¿\n7c?Q)
ÒÝ?X"¿\n7c?ïޛaÆ«?yÙÑî?p²qÆ-®´?yÙÑî?ï°èi³¡?…˜6S_^Æ?ƒÅå¾:¿?…˜6S_^Æ?ïΕ0B+ã?_ø‹"M©Ì?xµgö÷R8?_ø‹"M©Ì?ïòº£¤?^¹1Bè±?ZŠ¹eg'ø?^¹1Bè±?îÜ°ÐËg¦?°
>¸ê›?¢4òñ'·ª?°
>¸ê›?îÒçŽD&?œàò`¿K?¢ÞтÐ:§?œàò`¿K?îó+^þh?Ö9êr@? Î-F }'?Ö9êr@AGN4FGL J2324.6+3115?ÂÈ[Ó)LÀ<^ê–À:r®8(eÀ;÷|Gy;U@=eP@¿R%fÁÖ?Л™ðË/?ÒSû)×iß?ýu©dè·å@	Ñq§"=?íïMËdíÀ¿ãƒ!ˆZ¿êªó^1
¿¿îBÜ¢¨6¿ð?ïÿ~‹¡3UNASNone?ïú®aI=ƒ?Hjº"_?EFzx4K?Hjº"_?ïë÷S¢Ù"?iu&eùé?d¬b¦=Ä?iu&eùé?ï4͇æFy?'~TX÷?™fObà?'~TX÷?ïí(mÎ?Nµ'Oà9	?bג=ѽ
?Nµ'Oà9	?ïý/+ÍÊ_?D»=³ÇVI?6†Ÿø¨Wˆ?D»=³ÇVI?ï•/ü`Òí?"´Û)áï¬?Š´ÚÔ¹?"´Û)áï¬?î–\ؕz?™½Êÿ¬ÃÏ?¦Ÿª5
]X?™½Êÿ¬ÃÏ?ïý«"?	>&?¼àZC#ˆ?	>&AGN4FGL J2326.5+8555c¿×n'×E²Î@7Q¨½#žÀ:²š'^À<1¸£J"@Ä5Õyï…@Vü9¡â?Ìu‹‡ÞY?—½"]?Ǥô^@LÓ±Ã\?n'§¯S¿éTký@¿é'^ÿê±d¿è›ÿ/p0¿ïÿ^Ê¾?ïõl=ÀÕÉUNASNone?ïû¢ª±¼H?C$|øù?AuUˆe=?C$|øù?ïô;M€]Ö?_Ïo°ç9ó?W‰e(¤F?_Ïo°ç9ó?ïؘ:	?q‡ +±Å?s³âåüÀN?q‡ +±Å?ïù´$Æo!?7×ltÌ	ç?I/m#®?7×ltÌ	ç?ïúâºõ9?H©êŸT+?Du 4º?H©êŸT+?ïÃ×AÖö?ù"‡åE?~p"TÄù?ù"‡åE?ï½è®Þ,ú?iölò^?€…ÔCMWƒ?iölò^?ﶍíá;ç?v:¡Ür(?'\"ÉìJ?v:¡Ür( AGN4FGL J2326.9-4130¿âê'æ›ÀPàñ€
À:h8:Ùð¢À<À>-b@D³'>0'@A–EQBé?Áy}Yò吿™hüe85s?ÒӌDÐ@¹fM¼ÌO¿êƒ
€òç¿ãz–~ÜÿË¿éI‰¶Í‡¿åç¼r¶¿ëÈorŒ¿ïÿûbâMhUNASNone3FGL J2327.2-4130?ïòeÑH»
? +°¨–ñû?[4]vÈõ*? +°¨–ñû?ïõ{ëfs…?]½¦j•¦—?U)-™•ç?]½¦j•¦—?ï±ÍöÿŒy?"_Ìe0c?ƒŒ'Jëº?"_Ìe0c?ïþl¶¦^"?ÂQ÷sÁw?)4'}X ?ÂQ÷sÁw?ïû'©p°?S‰s=…¸¹?Céöã?S‰s=…¸¹?ïØ;55@ÿ?|º$'}?sâeT1t[?|º$'}?È!Êß?‰lÌÔPò?‡ÛNÜM?‰lÌÔPò?ïóÜ °WT?P Õ	˝…?XG¾úÓ?P Õ	˝…AGN4FGL J2328.0-2557?î	"õÖåÀQÕ_þmXÉÀ;V"tnÀ<撐Ü\@+È%Eá?þQ¶á¨üä?Û¾ó'ªi?ÐSX!+¯?õF‡nêÍ@v>Ôüò¿íº¸˜baõ?ïŒ<"Í¿åCá9Ñ]¿ÃžÅR…¿éñk}&œL¿ïøVž`3UNASNone?ïö®
Ò?PÒ:¸¡;`?SÀ£ñy»ì?PÒ:¸¡;`?ïç"M¶Rs?sèw'(rë?hl²‡†"…?sèw'(rë?ï«£ˆlô?}>>®×è?…äþƒ?}>>®×è?ïðZ+M>U?I¨'3ݵó?_K¨òvð?I¨'3ݵó?ïêÁï›{>?bçÞÀÿ÷?e>¦}B?bçÞÀÿ÷?ï‡Op'ɨ?™ŽŸŽ§Ø_?Ž,#éLþ?™ŽŸŽ§Ø_?ï:üOò0´?'.]ùiê©?˜ vq·n?'.]ùiê©?ï¿ô>M:?vâ{¾›?€ðo5'?vâ{¾›AGN4FGL J2328.2-4422¿ä‹V	÷ÑÀP€^"ð•À;£Ÿ}ß(ðÀ<ôy2?@ mnžÄ%ß?ü4 ½¨?×?(ßÈ'!?ÃCºió¹¡?ä{PÙ6h?üZËE8Ch?ìH‹¿¼C¿î:a?µøu¿Ïßü?Eö¿ÊrÜ@ˆ0¿æršA4Rÿ֓V¿)vUNASNone?ïm\¿žú?ÀöV ÿ?'Th|´?ÀöV ÿ?ïò‡Ë÷÷?_Õ‰9Æf?ZÄð.V¢ ?_Õ‰9Æf?ï×ÏÊ®œ?Üò`tÃ?t•
öJ?Üò`tÃ?ï÷Ž)§L?7ꈿ"§?Pâæ0¢gz?7ꈿ"§?ïýx؝ª9?10ÿÇ^=?49=,Wy?10ÿÇ^=?ïÐ>À–D?'Ò|^RJ@?wðà¹Ñåì?'Ò|^RJ@?ïÏøzÇé°?tIŽ–?xÂ{¾Óí?tIŽ–?ïâÑãPá‰?_ÈþÁ¦zì?m.¾<¿6?_ÈþÁ¦zìAGN4FGL J2330.5-2445¿ÒW ±.lÀQì<âž4À;,|CG}À<}€úfc@a.ŒZkÜ@™HUÚ'(?ÜA?Õ6ڇ rÒ?óšÞ¨—c^@I¤
æÈ?ïúy¾\òt¿ä '+"Ø¿éÖ]Ú¦ª#¿æñhÞë0¿ïÿ%¯¼ñ?ã'+ìíÕUNASNone?ïÈÎýS¨?zÚªZö?{ðe)`?zÚªZö?ïßçðzã?†>h6?p×,$¶?†>h6?îì¥Gw¸É?'KZÀl¡|?¡5«Š<Aj?'KZÀl¡|?ïãîµæèh?Uö…/bÄÊ?lJ@ó¯?Uö…/bÄÊ?ï sQu,l?xe[=W=?‡ã+'†Ù+?xe[=W=?ïCÒEeBƒ?¡Œµt#,?—…·Lxw¸?¡Œµt#,?íò¼iÁÿX? [¸‹4B?°j°¦*Á? [¸‹4B?ï/(
݅¤?‹üÚ[«¢?šþG¾çy?‹üÚ[«¢AGN4FGL J2331.6+4430?À‰Òž•NÀ0Q ÄeÀ;]ŒÁDŽÀ<À I·@ í;ÃO |?ý|s%³?ÑìoíÏ?¸N
áÀB?ê–>€nOi@Œ.'ã³?퐜ýç!¿í=äÒ}ö¿ÆÜ@WV¿Ù¿Ðºíý¿Ôÿ¶Äw¾¨¿å/uK¸UNASNone?ïþÖ±kâ?ñïXIÒ?""éˆ=á?ñïXIÒ?ïój–ø?`v­™žQ°?YÉ,/Ý?`v­™žQ°?ïõ¿{;Ƽ?V@ÉO

?T	\wˆ£?V@ÉO

?ïö®øÑb‰?6ŽºQ?R¢‹õžS?6ŽºQ?ïÿ#9sœ¸?¡càDL?˜Ú	?¡càDL?ï¾çìãÉ?‰ü:™F ?€FÄOm®?‰ü:™F ?ïú"d?\wí)h?G‰îþ"Tï?\wí)h?ïÞ±¯Ì4?`ô²BR¢õ?p§(.ç?`ô²BR¢õAGN4FGL J2336.2-0715¿âgé܅°ÀO§'`4PÀ;Š†‹ŸÛÓÀ<Ë+M‹¤@L}Dú0?ù>³†ªª?ßV·à†=?æƒ4õ«@àÎ&i U@þÎ4Uó¿îWS~WHç¿îùXG"©?êïàªÐ#¿ß2Š@ṿïÿÿ)@k*?î¸"†<ŃUNASNone?ïõùbƸz?€¯Ï»'†a?T
:ÂEú©?€¯Ï»'†a?ïìö9œr¬?fMfÉ6b?c	Æ sù?fMfÉ6b?î™ÂY#? Ú$áý/?®†o§J	Î? Ú$áý/?ïð²æO]i?RÚ,:=b?^š3Š€}è?RÚ,:=b?ïûÎxژy?W.ÙÓº?@Æ&'$Ÿ?W.ÙÓº?ï¤íÛþ9?EÌèÑe8?†Ä‰19Ï?EÌèÑe8?ýaŒ"?žs]»_ ©?§‡p)P¼?žs]»_ ©?ïÜks@"p?oãógè@?qÊFB)$L?oãógè@AGN4FGL J2336.9-8427¿î­˜‰E°ÜÀ@.0Â?«À:ú..çtÀ<'äö=ö@Ձšt_ù@GÂÀð ?ÅsŸÊ`5ö¿ŒìMñz&?Çf™	Ñ»@~+±Ì?ïÎ5Lèæß¿áV8ñ¹`¿â´1?¾¿ækœ 1£¼¿ÖI¯áÚ{¿á,$€èȬUNASNone3FGL J2337.2-8425?ïý$ß³Y?*øÙM5v}?7F×õք?*øÙM5v}?ïõpG:Ò?Wš—ÔÉ?UqfŸô3?Wš—ÔÉ?ïîb|T—å?\Yi«´á?aƒìÂ9?\Yi«´á?ïû&hŽM¥?)ׇôÕ!T?Cf^O R?)ׇôÕ!T?ïù@c"ñ?C8ߋ›Oì?JþsíÒ6?C8ߋ›Oì?ïÙ7ksä?{•_©¯û?sdJ1›fJ?{•_©¯û?ïçS̹_:?s""‹%v?h¬3u[ui?s""‹%v?ïç<ƒO;Ž?Z,€¢`íH?hÃ|؟ê?Z,€¢`íHAGN4FGL J2337.7-2903¿ï˜çóÍJTÀRiIùHUÚÀ;S·K[H%À<Ìzü ¯@Xs3©P?úØ»'øme?ÚÔ"Zï?ßwç˜*-Ñ?ú­êk|?öY<tz{F?ïK;½›Vˆ¿ì$2å/š¿ÓzcôF8¿Úƒw
S¿í×Þ
fðÐ?ݹÕcÊ)ÚUNASNone?ïÚ`U¢–?š;;¥{L?Œ‰gç'¾v?š;;¥{L?æ??¡çÊ
Aû¸?˜¿p]?¡çÊ
Aû¸?íŠþ¡¹¬<? €W¸ª;?³¨
ò 'ž? €W¸ª;?ïá•Ü ª?…©.½ À?œãÍMð©?…©.½ À?ïr1\ˆ/ÿ?'{û>žM?'¹Ôt!j'?'{û>žM?ëÉèêÒ?ÈÃäÈäWO?ÀØ\Wĸ?ÈÃäÈäWO?íŠD«ÅZ?¢Kdq2Œ?³­Ú£úñx?¢Kdq2Œ?ìGýr\û?­@ß#~™À?½Àmh%?­@ß#~™ÀAGN4FGL J2338.1+0411¿ìúÄû$׃ÀK©~+VÀ;LÓî)>À<}3+¦w@!Ž:´w?ü/[7^;?Å1'Y4?"Ó= ¿4«?ÀÚA?Šb@§ákv¿ïÿÿ)@k*?ïì¿B ?î¾}=B¿ÖyV@!-¿ãi¬}Ãû¿ê!ۇz³%UNASNone?ïÿ9=…¾é?Šêò¾¾É?ØT¾·@?Šêò¾¾É?ïîmaéeE?dñÊ9ÌãÊ?a'å [5?dñÊ9ÌãÊ?ïë¬s»är?qÑ™œ9U?dSŒ
!Î?qÑ™œ9U?ïõµFHcÇ?Dk"¾b¢Ÿ?T•st·Ò?Dk"¾b¢Ÿ?ïþÖ+Ú¤?]Y6?"ž>ßÀRN?]Y6?ï±as¯Ç{?ŒGÍfS/Î?ƒ§£ l¹<?ŒGÍfS/Î?ïë!½¶–?wZ1?dހQg²\?wZ1?ïòïJÈr—?T¨nLz‰3?Z!j$ѝ?T¨nLz‰3AGN4FGL J2339.4+3008¿ÔºL[gµÀ>2É.4À:Ô®ôt±ƒÀ<Œt¬zFî@ Å#
F*?ÿ=GþœS?ËW+ lÇ?¨Ó7Â[|?à?3¡íûñ@°Ø–¯"h?ïڍ¯ãˆ¿ê¯À¢r¿âd2å/š!¿ÊU½â#K4¿ëb¿è¸¼?£o—ß҅kUNASNone?ïúŽ8^ãˆ?;PR§Î}?EÇõ'"X?;PR§Î}?ïïÜÛ‰?b_B¼XWz?`#$¡bÏM?b_B¼XWz?ïÑI´)ò?uS…$¢å³?w[&
#2Ä?uS…$¢å³?ï감´¡;?JTÚOOÊ?eOoA¿Ý?JTÚOOÊ?ïûG¬fû¸?= ˆy—"?BáM™4ÿw?= ˆy—"?ïÁÏ­Ÿ?ˆg¾ìj?~vøŒÈ–?ˆg¾ìj?ïÖz~)b?~Ø	C¿(?tÂÀËáç"?~Ø	C¿(?ﴛK(%?oH¼#]°?'Ù-(@¢?oH¼#]°AGN4FGL J2342.4-4739?Ê?º[—;­ÀP[Æ?À:¤;ðqÄÀ<´;4‰tˆ@žÿãO›?þŸS‹˜O?Í)ß!Ž?Öû" áa"@Öt_Mmq?ýÃwÌ?^:?ç"ÕåzB¼?ß®3Äþw?¿â§'A°¿àáA=â䑿ïÿþR€ÖT¿®O×®¨˜UNASNone?æs.èÃè?Ê>Á?|?Ó¢.yÌ0?Ê>Á?|?ìàÏPé/7?ÁNƒøì«?¸ù…y'mI?ÁNƒøì«?æZø6]	E?±»ùZj?ÓJ"Eíu?±»ùZj?í™ÖqÕõ?™ç¾ðÞ?³1Lq¾Kd?™ç¾ðÞ?Ó•+9®f?ÈÞ©Õ7;?æqµjc(Í?ÈÞ©Õ7;?Þò=ŒIò4?Ó§u3w•}?à†á9Ûæ?Ó§u3w•}?ÏÚ( 2:?³G8K©H?è	u×óq|?³G8K©H?âKäy´m?¼SþãRþ³?Ûh7—Ï%?¼SþãRþ³MIXED4FGL J2343.0-4756¿ÚBä˜Æ`ÀPR§Å¬À;b¸N†ËÀ=¥O°A@ ´ió
Ô)?üÇà"9¶?Óã=ñ?]ðv@>†TBw@²&|–~‡¿Ô×ûØð?Öß?–¿do³Âض¿ÃÑe¸Á}
¿é_9ìŠØ6¿ïÿü9¡â=UNASNone3FGL J2343.0-4748?ïȏ«þ?ˆm§ø
?{¸@vYLô?ˆm§ø
?ï¹°^hQ^?Û&bÝsM?"ètX?Û&bÝsM?îå!çÓ°¹?"í%7Q?¡­á'Äôo?"í%7Q?î'2Ђ?•®¡:8:M?­Ü↬ß?•®¡:8:M?î<À'3ý?®¶ƒüwªô?¬3÷á.?®¶ƒüwªô?ïdzQïz»?¡Ùz*ª?"pµÀXڔ?¡Ùz*ª?ì1á¿Ö¢Â?®O§p'|?¾pòJéï?®O§p'|?é³ý¦'Ì?¶'C©·™Á?É0	gÝ´Ò?¶'C©·™ÁAGN4FGL J2346.2-4322? Ö%QYHÀQDÜ3rTÀ:ÝW4šÀ<§JNØ«'@ýG#Õó@	q"Úí÷À?ü]ò#žjº¿¤¹OÂ`Z?ؖ;`~Dÿ@…ê⣿Ò`£üž÷¿ížo÷ß ¿âqáÄ«–¿î©;,ü¸M¿ïùL`RP?Ë,b^™éKUNASNone?ïÛa48±?ªcعâ[Í?rOtçókµ?ªcعâ[Í?ïë
l­±?ÛDŒ?dðòUyWz?ÛDŒ?îI³rˆ³˜?£Ú§V˲©?«dÈÚäbw?£Ú§V˲©?ïý°+}v?*s`,ƒ>x?2{õ'¥÷ì?*s`,ƒ>x?ïþoÞ£þ'?<_V;ý6?)ÙïÛø?<_V;ý6?ï·*¶âÕ£?"xYQ+Ëô?'5RP9"G?"xYQ+Ëô?ï6$Õ!…?•+k"¡Ýá?™;edfd—?•+k"¡Ýá?ïЀh®¡?zRÉ;øȌ?w¿ËÚûãâ?zRÉ;øȌAGN4FGL J2347.0-5720?ÕOJ×oÀLÚðZpŽÞÀ;‹¥·µÀ<ã?«çy÷@ö¨M'ƒK?ý ìt2?Úy¤)ëa?Úøäl-P@ y¢ƒM'@<!Gxd–¿ïü£ŸVòÖ?ïÿD¹mtx¿Þ¥¿'6{'¿ãkŠýõcÅ¿ïÿöût€?î÷ôÎs•úUNASNone?ïõ8ša{×?Wî‡Dó?UŽËqBas?Wî‡Dó?ïòšžC"?bsm~ì@Ç?ZÊÞüG?bsm~ì@Ç?î¦ œòXf?""Я'oØ?¥ö-jݟ?""Я'oØ?ïõégÑå)?CéAa‰?T-0°
?CéAa‰?ïç‡701»?nY£íÞ?hxÉ'Üà?nY£íÞ?ïÄ"~Úüe?‡i˜Qþ¢?}îÀ~"f?‡i˜Qþ¢?íž*aõµÇ?¡ù
'ÈÖO?³¬ïwM?¡ù
'ÈÖO?ïÉþy‹B?qçÏ'lÓ?{÷ ÞFó?qçÏ'lÓAGN4FGL J2347.9-5106?¿(å–6&œÀO–/­lµ5À9£OÄcq¿À<j1ßv½@s€Êë¡@¢%ߍ™±?±X¯ïqgv?¦î2ß6—þ?òDÊÕ{Ç÷@"_õ3d¿ÞÉë¼&6v¿ä&Ë4*ª¿æ`C¢?Ý¿çzȞü·¿çQ	<¿£ï¿ïþ SUNASNone3FGL J2348.4-5100?ïÿWä?¶ÿÜÀí2?ý<_ÔÚ±?¶ÿÜÀí2?ï÷˜â?U`[Hã?QæÍÛ¾ÍÉ?U`[Hã?ï﮳ ;?[àÃXh¤•?`QLÅ˼°?[àÃXh¤•?ïÿiH)J¸?»!K‹<?ÖöQO´?»!K‹<?ïÿ] *¿?ɾ¢õ?\‡¢Ô°Ñ?ɾ¢õ?ïÝŒ†á†?xawl¿›?q}9Êý˜à?xawl¿›?ïèNá£1?mR«m´gì?g±·£_^?mR«m´gì?ïþŒ³4Ô?!rß¡Øþè?&÷1È×Sÿ?!rß¡ØþèAGN4FGL J2350.5-3930?ä†]Uh	ÀR.bÀ;XLpñÚ£À<Ç$'&µv@ö‰QLù®?þºƒ-?ÚԎ!ÁEÛ?ár×Ã Ô @҉T§ø?êIWÚ(ø>¿ïHðŽ?ï`?àÓ¿ÍBjCk¿èé£Ò؈¿ïÿs+(x?ÕG$ARۚUNASNone?ï¾#}CÞ¸?§ŒLöpÂ?€w ­¨yñ?§ŒLöpÂ?î={ÉOä?¶¸Ñ²k Ù?¬(ClƏ·?¶¸Ñ²k Ù?퇵%!D?)L¿?i?³ÂWDé_?)L¿?i?í¬ŸB|…?œ³bK,VÔ?²›ðeöW?œ³bK,VÔ?ï¾8ú"Ó"?‹£Ñ[æˆ?€qÁ[#?‹£Ñ[æˆ?ä°.l,¬?Ò¨ŸlcÎ?֟£'¦¦â?Ò¨ŸlcÎ?ì˜×6Y??¤=:µ`?»9GVM6?¤=:µ`?ãOo*Žn?ÀÌÒ®/ #?Ùa!«Ôã$?ÀÌÒ®/ #AGN4FGL J2351.4-2818?æú*ÀS+à`þG™À;&ˆ|:äÀ<¸¾ aŸW@XŠv;³@ä®ZZ?ÏÆ_u;@?¼§0ž-}?êŽSz
ˆ?÷àO"'é?îa.¹Pï¿æúf=v®¿ã.^œîc¿äîV,\¿â«={
¸¿ïÿþøþ"UNASNone?ï÷h8<vB?R àx
à§?Q/sÕ¬œ?R àx
à§?ïµD¯Ô»Ñ?œ_ß5EŒE?'®Ô×­²?œ_ß5EŒE?®pã?‡AÐÚÎm6?ŠÔ"\çä5?‡AÐÚÎm6?ïÁ ]®?fj+fÖ?o·æ¾<õ?fj+fÖ?ïõ)–ì?XMñs¡íŽ?U¬ÒHô"ð?XMñs¡íŽ?îƒax.Õ?¶\ü~l÷¸?§ÏÉê4à´?¶\ü~l÷¸?ï:´ÑzÓÓ?•ߪÉ8?˜©eÉÆM¦?•ߪÉ8?¿4w›?"W
žrH?§…¸W?"W
žrHAGN4FGL J2353.2+3135¿ÓjÆÐÀ=ªV¼¥7]À:Tð=ëÀ<JHêT@u1æ,@Ø'sâP?·ûø‰iÔ¿§¿6a;a?ív+57ð1@	WS\¬ÿ?ît=¿~0¿ç2–À¡E`¿è~=½Ð°‡¿ÞV`x»þ¿ïÿþBe«+?ïÿì´É ÈUNASNone?ïûè#òw?8)Ų—@P?@_rΘA?8)Ų—@P?ïò'­ÌŠ?`ôòØ:™M?[°¤¦$°Ñ?`ôòØ:™M?ïá&À«x·?q£¢˜,q?nÙ?B©Q?q£¢˜,q?ïúÕà¶}o?1¹³ð…K?D¨~6¸é?1¹³ð…K?ïü6ýö™??‰áµ%?>Hi¡èÁ??‰áµ%?ïÇoJ,'?…Y«ŠÍ?|H[Ç"?…Y«ŠÍ?ïå0œtj?u˜ª9©_?jÏêL.=À?u˜ª9©_?ïÝßê5éF?cTč÷?q
ýȌÞ?cTč÷AGN4FGL J2355.2-5247?äPS]'×ÀO#ãŸw),À;žUÀüµÀ<ÁÐ%Fáf@‡Ü¥Aî@[ˆ^Þ²¨?ɕµ‰dBJ?à…°ÿì·@,`RP/@
.'uÏ?í#P!U*¿ÆbK#¿Í¶¿à¹*ù¨Íê¿éþqTÖñê¿î[ÛÞb¡`¿ïý󀕼•UNASNone3FGL J2354.8-5245?ïôØb4Ü?'yWÀíVÁ?dõq2}?'yWÀíVÁ?ï×±&"?}Êsw?t'8h#Ba?}Êsw?ìc'\*Ş?¦%+nÔÛ?¼ãu©Ó?¦%+nÔÛ?ï'LŒ±ºß?p¨´¹¸wp?‹¬ÜÚp€D?p¨´¹¸wp?îLwç1æ?«åxßø"?«8'V–?«åxßø"?ïjéæ8-Ä?›†ÍÐ]?'¢Ã7By‡?›†ÍÐ]?â<‰G"a?¸è©ú1V\?ۆíñp×??¸è©ú1V\?í?¶­aÞ¨?žÁ»À˜³?¶J•^þ;?žÁ»À˜³AGN4FGL J2355.5-6614¿êD\Þ¨A}ÀHøSX"À:]RtA}À<Zºà;>š@·Â«ášº@†÷ µí?¿¹? §??ÑO9c£éT@Ñ ;tJU@"é3_ÓÐ?˧9ÓtÝ¿Ýë®ÄùäFfގ–¿ê–—Péý_¿ï‰nÿBž¿ïò
"þ2UNASNone3FGL J2354.4-6612?ï†5šì€?'²8±S?Žx²§Oñ?'²8±S?ïݒéëÛJ?{¼ð£!í?q6Šë%ßU?{¼ð£!í?în7["?œ^"€;?©ŠR¾c´?œ^"€;?ᆭf[©Ÿ?c¿û.Fa?€VffUèF?c¿û.Fa?í7Ògô?³wóvÚ§×?¶Ao\Rh?³wóvÚ§×?ïjpÃa"? œU7tHm?'¿Ñä$1'? œU7tHm?èÝ &?´;R®§?ÍÀ‰g‹¢?´;R®§?î_›AB9?"äL7"€{?ªKïMÈc?"äL7"€{AGN4FGL J2357.8+6839?Ѐ²Y¦[ì@/çáüúÀ:{·0ƒVÀ;'²´ҟ@EóH6¦@
äÏ©?Çw¹…_?·oóegä?ñØ·lwÒ?ÿ$SÚÁ'?ìÙ]ÔÇm¿à²Åº‰Ô*¿é…¡êöÙ¿åá';"¿ê8'üÕ©¿ïÿèž:UNASNone?ïà·Bvòü?jrihâH?oH½,Œp?jrihâH?3æ}?':úS£?Žs:Æ`³?':úS£?ï|öz	R?".fmÆ?a0Å»M®?".fmÆ?îÔ'½^ž?€÷Rµ½?¢½"11ä?€÷Rµ½?îQÎÕ̶ä?¦°WFwƒ?ªã  ÜÊ?¦°WFwƒ?ì ½œ¥Š
?ÁBd/É2?¾úÓ¯¯?ÁBd/É2?ìÛ$"
?§/¤J‡®?¹ã&Þ?§/¤J‡®?æêd¢8q?¯ïlþ¾³ñ?Ò+6»ü?¯ïlþ¾³ñAGN4FGL J2359.3+1444¿ämó¬KÀG ÌݓÄnÀ:ÌhfçÀ<tlâ˜@êx»}š@MvûßßÏ?ÖÒ~ýáí›?ւ[Ü®l@` Ùÿ»7@rX¹TŸê?áhÝ{µƒ¿â9
wt¬¿ãØîª_å¿ì$4'®ÃÍ¿ïèè¡¿'â¿ïûÕctCŸUNASNone?ïùnbֆV?CÌYÑ×Êi?JFuBº?CÌYÑ×Êi?ïä3jTvi?qîX¸PÝt?k̕ÞcÏ?qîX¸PÝt?ïy+‹VØ?ƒfό)¢?ÚŸ7,*ð?ƒfό)¢?ïÂT_•"?bpM9«‡­?~Õ¸H¦Jú?bpM9«‡­?ïóëw\ØÉ?[ƒñÓH½5?X)}H-«?[ƒñÓH½5?ï"-¿UëÅ?'Ê™ó"è?‹4*…È?'Ê™ó"è?îâ
cb?—ZX&ŒÐ–?¡Þ/þMâÝ?—ZX&ŒÐ–?îŽÓÉ?ŒÃ©g ¨?£¤"̘%z?ŒÃ©g ¨AGN4FGL J0429.0-0006?ï‰<"€|À?BÝHE0À;*šÞ=8À<!-••@j/Úc8_@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ÒûÏ×g?îuU9y¿é‡V +à¿ãý…Â!M-¿î0£kªs¿ïþx«ãH9¿ïÍ®5öAGNbcuTXS 0426-002?ïüِ»µ´?@)'D}$?93zHÍü†?@)'D}$?ïûúÖåb?`ßò"ڐÿ?@¤ïw³?`ßò"ڐÿ?ï!·F?ƒº38*ښ?‹÷''Ck?ƒº38*ښ?ïõ~-Ç?<q¡–hZ?UÛö̪±þ?<q¡–hZ?ïýG¬š…Û?A.ð?5™p¶ºø?A.ð?ïïéù>«ó?‹•œÜZŽ‹?`ÁT‹?‹•œÜZŽ‹?îÆ÷'>]?™"ÝñLï?£žPŠøe.?™"ÝñLï?ïÐ(à–P?j×od¨%m?wük‰…Œ1?j×od¨%mAGN4FGL J0534.5+2201i¿æD&v|cÀ <Ž%ÈÀ5ì"ÓiŸÀ;˜=)HÏ@"k±»¤[j?ü?ȔhqH?´zá?òõ†@íT¬ª˜?˯¤Gó_¿°^WàL퀿Ð9–m•/¿ÈÙ
¸OgF¿Þ:—Àü_¿Åa2àRÂOTHERPWN3FGL J0534.5+2201iCrab Nebula?ïÿUë;o9?vÛžÆN?B–Ñ
›?vÛžÆN?íÛN6çC?É!êÅG?±%ŽHÇ]ç?É!êÅG?îÖ×g°h?¡W+~ì—?®Ò'†ñD}?¡W+~ì—?ï¶_s5µL?ƒM2èâŽ?'h#=ébä?ƒM2èâŽ?ïþÒþa'¸?$Š'¡|˜?"жâôZ?$Š'¡|˜?ïY|JÔ9©?º´fÜOn?"ÐvœáÄù?º´fÜOn?îŠûàFãP? ÛcñõƒÙ?§PAúµä	? ÛcñõƒÙ?ïF\@{MÝ?¥zõçé¬Ù?—4wð–Di?¥zõçé¬ÙAGN4FGL J0850.4-2558?ÙܝUÌ÷P@&Å«ŸU›=À;CHdàÀ<Qpنïs@û&s\æ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ùwy‰-ç¿â'¡Ã3Æ׿ìªÒ ɤ#¿æÖ¡aä÷f¿Ö؉™qV¿ìŒ$ÁUuR¿ïӜ_F·tUNASNone?ï´²
	?'ÿKë?	iÀuìå?'ÿKë?îkQ,mqH?±LCËKâ?©Jí8Mˆ?±LCËKâ?îúЗBãf?"èv£)Î ? RöL ?"èv£)Î ?îÖÞ0wl?…]Gj1?¢'ûøÚ(?…]Gj1?ï@ÏÜP?Ÿ­¢Œ·Õ?ŸwåýÞ?Ÿ­¢Œ·Õ?⨺b«µ•?Ô{&hÝF?Ú®‹:¨"×?Ô{&hÝF?ìu b'ù?¬CKCË0ë?¿ôRüëè5?¬CKCË0ë?çÃÔ¢üf?¸˜d²©'g?ÑàxVº4?¸˜d²©'gAGN4FGL J1039.7-1540¿³0TzüVš@BKl6KìÀ;/æw˜¾À<Zíl…@[öëYTÛ@θ`?ÓÀ–?"aï?Ån¿³è-?ñéÿ¸‡p@Âë'D"X?íãC ¼
7¿ì'lá)Ñ
¿ãÇ=áâއ¿ïŃAéYu¿ïù™ê!qj?î"Nü½UAGNfsrqPKS B1036-154?ïÿj‹[Š¸?'r®
rS?®'Rò¯?'r®
rS?ïäa­*VQ?'RÒ´ef?kžS£n³?'RÒ´ef?ïº^Š׸?×(8ú:?h]}±Ì?×(8ú:?ïô4*‡›ž?@
ú‡ ?W—ª®ÐDŸ?@
ú‡ ?ïÿ¢¯dS‰?Éׅ"ä©?T+ÕÖJÉ?Éׅ"ä©?ïääFï†?‹½ñ:J?koõ‰™n?‹½ñ:J?ïqì‡ò?_Ð:¹'?'Â~e¸?_Ð:¹'?ï®ée<x_?w+U:¼a?"E¦¨úÎP?w+U:¼aAGN4FGL J1202.9-5717?ÝÍt
•e@ևà3±ÞÀ:å¼dŸ¼ÉÀ;É>adžæ@W=Œ¨ou@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ZRúMäd¿çëe>H:?ﳫ=°å'¿ØÎªžœ¿æébßôñ¿ïÿã_¶Hý?á±À6UNASNone?î©Loø¾÷?·Òc="¾¡?¥k8ýà[™?·Òc="¾¡?íH›%qò?ÂÊ\eÔ?µ»&ÒQÆò?ÂÊ\eÔ?îÂsoa?›_^sùƒ?¯ƒØÐ×î?›_^sùƒ?ïè^<?'Q*¯Ëô?œbï?'Q*¯Ëô?êïðøÈu?À×¢~D©}?Ä@<Þ)Ž?À×¢~D©}?å"»ì¢?Ԕp{ú3?ÕâÖàˆ&¼?Ԕp{ú3?åAÒÓw?¸Û/Qpç?Õ|üZYê?¸Û/Qpç?é.«Ê*[?µ´jì%{?ËESü×V"?µ´jì%{AGN4FGL J1209.9-5923¿æŒÀW?ú8@o¬)ÜrÀ:rrÓ\3À;<¤'D`'@k$†r'@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ø¹µ‹g§¯¿ï,,À/[?ïõ0~Mù¿ãj–â/4¡¿îÓ¬àsGË¿ïù'm-*¿éê•ÀF+³UNASNone?葉ü¾hA?'G\Áê+?†"@ÌöS´?'G\Áê+?åÆá§`'Î?Òr¥'í?Ôr<±>Úd?Òr¥'í?í#}®+¡ï?¡o=ÓÏl?¶äŽ¢ð…?¡o=ÓÏl?éöj	Þûù?¦ÿì0€«€?È&W؄?¦ÿì0€«€?ë¦5w
Ü?ÀÏr÷÷Ñf?Ág*#ȏ¯?ÀÏr÷÷Ñf?Åp?ºø[h?̹v™9wp?ê£ðAé&?̹v™9wp?áÐxN¬qŸ?¹l6.ò#?Ü_b§Ã?¹l6.ò#?Ñ÷ú659?¼×Ú$¬»?çä¿ed?¼×Ú$¬»MIXED4FGL J1320.5-6256c¿±åg'2r9¿Ð¥é^'þwÀ:Ĺ­À:ÃM~8D@!XÒTÌ
/@…Áÿ¿=m?Ù6>`7ù?ÑìD`Eÿ­@=جÔà?æ€á;ïÿªÛ
}2?ïôßÀÅWŽ¿ÛàY¥"¿âr·bWc¿ìp	è·UNASNone1FGL J1320.6-6258c?î
'bðe-?¾G8Æ"?¯-‰ÐÆ,?¾G8Æ"?ï_—¸¡zA?¶LüHj›ã?"
ðø!Ñ?¶LüHj›ã?êÓÅ7#¥?¯SÆ1ÅMf?ijÄë#ql?¯SÆ1ÅMf?ï—ÀÏΤ?vb5Þjû=?Šù–[+?vb5Þjû=?éõ"ø¤—?Äæk#i^?È)³˜m¤?Äæk#i^?ï	ñoæº+?Á`ˆ"?žÁÑüI'¤?Á`ˆ"?æùʽ(c?¶*ê¸þ¶??Òj"á¯;?¶*ê¸þ¶??íàüƒ?¦çöeJÓ%?°øè»V2?¦çöeJÓ% AGN4FGL J1622.8-4454¿Ö9=u£½@
ß_ü¿ÙŸÀ:?íë*…æÀ;I6_7ü@³›õ>…ø@uuf͔?ÔÉ@v¬s?Ð~®?þ'U_­å?þìrtf¯7¿îîoÜV?ïþê‹út¦¿ë§žªz'm¿ÞJû܄е¿îñƒ€R ·?Áƒ-FŠ(
UNASNone?ïmçuUÔ?¬à±£T)?Ÿ²C|¯ƒ?¬à±£T)?ë§ùôx7t?É|˜¨"Ž?Á`."/?É|˜¨"Ž?í춽ýã+?!6>R–?°šJ4ÿ¦?!6>R–?î¼XÍîØ2?"s¹ÕÒò?¤:sÆùé?"s¹ÕÒò?å¿3S‹æ?́&·‹c?Õ΁™Xè5?́&·‹c?à ¥3xí?ÕÝ*K
Èä?Þ¾µ™Â&?ÕÝ*K
Èä?å%Áܔý?¶Â³éšñ…?Õ´|FÖä?¶Â³éšñ…?æm¶•&?¸ø­À¿?Ó$'Ôá÷µ?¸ø­À¿AGN4FGL J1758.3-1920¿îpÐ#]A@Àó°fÀ:³!*3À:Ì&€IR@!
²˜@LÌ?ß ?ÝF"µ…'?È5*ÀY22?úâÿýPÎ?þ3³P¤Þ¿íß/ûÆ?ïäÈÁû7™¿æ>Ê€Â2¿æû]U¹¿è?tŸ&ú¿ïÿæ4|ßOUNASNone?ì9XëöÖ?ÇkŇv?¾58 IOï?ÇkŇv?◧ÂãP-?Ótã^V	?Úаz9_¦?Ótã^V	?êDtnfåè?°/ˆýtr?Æî.Fdh_?°/ˆýtr?êNíSUª?­êÇ{Ø}*?ÆÄJ²«¹W?­êÇ{Ø}*?ݸá´v¥à?ÐzHvøk?á#%Ä­?ÐzHvøk?Å(…-9?ΫÞä@K?êµøÞ´¼ò?ΫÞä@K?âë¯u›Z?¸hM)%(´?Ú(¡ÉKõ?¸hM)%(´?Ë'ö°K?½W•Š¯?é;ö Sí?½W•Š¯MIXED4FGL J1838.0-0516¿~³¹ì¥y?áöѝìåqÀ8͘¢ù"¬À9ïœp
¯@%¶Ê×Õ@3€*?ùCO`Š7?ÖÞEvX³@"Jà£ï3@K¹•ãV§¿èîVŸÉß]?î8†ß'±÷¿ãý+-«4¿êÌ W"ý¿ïÿšŸ¨ý:¿Û
! á÷×UNASNone?âȁ4⤔?Ö.®2q±?Úný–:¶Ø?Ö.®2q±?Û[ø¡?Ó"[
†•?â|Òÿz/?Ó"[
†•?Ý¿B£ØQ?·>Ö[j)­?á }^®Ø?·>Ö[j)­?ãüfGݏ=?À7Òä¥?Ø3pDá†?À7Òä¥?μh¢<¹?ÕHVþ6?èPå×pûÒ?ÕHVþ6?­{Û÷Ò~?½œÿ³1£Å?î(B@Ž²Ø?½œÿ³1£Å?ʲ`ôÑ<?´¼áºs ?éSgÂË°Ý?´¼áºs ?µ9–¼²?¶ÊN`'ù?í_ØÍX…J?¶ÊN`'ùMIXED4FGL J1841.3-4442?â3mƒn½À1R`õäÀ;R`îWaÀ<{y¾Óæ@½›yÙ@¯¹À*§ô?Ï;˜@—ä}?­"@ fäÒ?ßrl@gpŸ@
Nܱò+?ê…cíbt?ï^JZƒÚ¿àiPüqÖ¿æÆÙmÄÿy¿æ˜y¾²Ø°¿ÅÁÂ<1µUNASNone?ïýX±62?. ¬ ßú?5?K3l ­?. ¬ ßú?ïøa}ÉY{?f0(ÊÎÀ?Nz=ëåÃ?f0(ÊÎÀ?ïäĪ-ï?gvF!Z?R?k;å,–Á5?gvF!Z?R?ïᇯêÇg?PCI»ëÀ?nxOé=™?PCI»ëÀ?ïù:™6¦?EP«:X•V?IËp1]?EP«:X•V?ïÑëÐH,j?›ž}÷*- ?w
Â|¯Y?›ž}÷*- ?ïÐZß'Jû?~áW$Rek?wҐm
nh?~áW$Rek?ïù'ëàÂ?{ßxã$i?Ï©c¼?{ßxã$iAGN4FGL J2048.4-2517?Ðq˄xJ?ÀBa$FEÀ;ž6a»Ü»À<Œ~å¹,Ý@rEêE@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?üŒ ŒÒáº?ÌWµž‡êð¿î·Þ"ž­Ö?ÁB‡dð¿êj˜Yþy¿Ðæa=²"¿ïÿÁKJ‹UNASNone?ïÛyúS)?uNáÖD}Ý?rCόF?uNáÖD}Ý?ïÒp[xÌ?‰ÀûÜzá?vÇÒWGYò?‰ÀûÜzá?ïs´¤{¹¤?ˆ¾PƒLy?'‰km/'?ˆ¾PƒLy?݈©)?q:³/ñÎ?‰'¤´íÂ?q:³/ñÎ?ïÂj™âûÉ?€âãÞ5þ³?~ʳ0.G?€âãÞ5þ³?îã$ݧ]?·Uï<¤¦1?¡Îý³q0?·Uï<¤¦1?풼øQó?¤wAì8ÁË?³j?Åpk?¤wAì8ÁË?íð'ùKä?©hwŒÏ<Ü?·è~¾ëÆ_?©hwŒÏ<ÜAGN4FGL J2106.9+2455¿ëþíFûùÀ-Ýãø¶À:êﲪâ—À<3¯Rhƒ@À0"eÛ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@	Ýä$g?ïÿÿÊPË¿â=zŸXub¿ê•ñ¤ª[¿é¡­>¼ÿ$¿ïü¤–LÝÿ?¶Ýßnºó±AGNbcu3FGL J2106.1+2505MG3 J210642+2501?ïö­¨¼™›?zµ!W?R¤®URiÈ?zµ!W?ï÷–F'r?qáË úi?PÓû
fý
?qáË úi?§CGË?…`µËŸd?ŽZV6
EG?…`µËŸd?ïïƒI\PŸ?D|Ïóî…Ì?`|¶•ðñ?D|Ïóî…Ì?ïùûK»?\?UÍPtœh?HѓfÞ?UÍPtœh?ïهûâd?šËRfc¾?s<ïá}H?šËRfc¾?îïÇAXÌ?–(ø­âb?¡‹ì+
ª?–(ø­âb?ï¸xyZ×3?rraj×Ðé?áá™Óõ7?rraj×ÐéAGN4FGL J2325.9+6206c?ïþ4ê "h?ëê*«¥4ØÀ9¼iVïSÀ:øqž¨Í@5ü+46=@¡ÿ›¬?՞ë@]ñ«?ÁœßÉw?öæó^ÜÚ6@xýz>µr?ç}ÈMKŽ?îq!ôœu¿ìz_í{n¿å÷QÕR¿ïö¸ÞÙ>Ë¿ïürAeûÝAGNbcuNVSS J232543+620829?íö«ËþÏ?ÇKÖ D]?³J¡ 	†?ÇKÖ D]?êÿ_Yø?Éý…ç¶9?Ä'›ü?Éý…ç¶9?ëõ
lPÇ?¦ãùw?À+çÖN¼ã?¦ãùw?íãÊßP¡È?'P‡¼SV?°á©2¿¿?'P‡¼SV?åæ&¯Rz?Ðd—f¹r?Ô3Û²¡[
?Ðd—f¹r?ߥ^(j?×o ÓÎãl?àq­PýëË?×o ÓÎãl?åh)v¾DÁ?¸6ٗÌ ?Õ/­ƒv~?¸6ٗÌ ?à?	D??½èò@î?ß߁íw߂?½èò@î0MIXED

==> SOM_VIZIER/4FGL-DR2_prob_catalog_2classes_SMOTE <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  334 / width of table in bytes                        NAXIS2  =                 5788 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   39 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\SMOTE\4FGL-DR2_prob...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'cos(GLON)'          / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Pivot_Energy)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'LP_Index'           / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'Unc_LP_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'LP_beta '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'LP_SigCurv'         / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'ln(Variability_Index)' / label for column 11                         TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR12    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'HR23    '           / label for column 13                            TFORM13 = 'D       '           / format for column 13                           TTYPE14 = 'HR34    '           / label for column 14                            TFORM14 = 'D       '           / format for column 14                           TTYPE15 = 'HR45    '           / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'HR56    '           / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'HR67    '           / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'Category_4FGL'      / label for column 18                            TFORM18 = '5A      '           / format for column 18                           TTYPE19 = 'Class_4FGL'         / label for column 19                            TFORM19 = '5A      '           / format for column 19                           TTYPE20 = 'ASSOC_FGL'          / label for column 20                            TFORM20 = '18A     '           / format for column 20                           TTYPE21 = 'ASSOC1  '           / label for column 21                            TFORM21 = '28A     '           / format for column 21                           TTYPE22 = 'Flags_4FGL'         / label for column 22                            TFORM22 = 'I       '           / format for column 22                           TTYPE23 = 'AGN_BDT_S'          / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'AGN_BDT_STD_S'      / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_BDT_S'          / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'PSR_BDT_STD_S'      / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'AGN_NN_S'           / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'AGN_NN_STD_S'       / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'PSR_NN_S'           / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'PSR_NN_STD_S'       / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'AGN_RF_S'           / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'AGN_RF_STD_S'       / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'PSR_RF_S'           / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'PSR_RF_STD_S'       / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_LR_S'           / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'AGN_LR_STD_S'       / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_LR_S'           / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'PSR_LR_STD_S'       / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'Missing_Values_Flag' / label for column 39                           TFORM39 = 'I       '           / format for column 39                           DATE-HDU= '2022-01-29T22:26:05' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             4FGL J0001.2+4741?ÙùË Q­"À,­º<§À;J,Rƒ[À<‡éÐ2@Qì̜{K@Þ¥šXÜ:?Ë·¢C6`¿Q¬gsùï?µz'Ÿ'h3@ù-@*¡¿ë8罓ô¿?讵¬ß¿á"c+YJ¿èÙE¡Iç*¿Ú!*•»¿Þ
\¿žúAGNbcuB3 2358+474?ïü­Ù:?=p=D&]B?;''6/'Ä?=p=D&]8?ïþ|Rñ¸?JÕ¬È7Ð8?(>*Ðä|«?JÕ¬È7Ð#?ïÅßýõ
?~^@tL?}y`?~^@tM?ïýHù$ó?)Œ'+ž,[?5¸7>Øi>?)Œ'+ž+ý4FGL J0001.2-0747?ÞÕGqçî~ÀPӅH©¼ýÀ9j8³¥´ZÀ<‡þ[@ŠÝÓÛ3î@"<½öp4?°Fc熝?¨ø\óvè?úƙ¬äÐ@ý"õ[?ïïXÌý¿á®?Ffí¿ã¤ÊOD
ò¿Úþ-b8Ú<¿èa~J2Կވ–<"AGNbll3FGL J0001.2-0748PMN J0001-0746?ïüL¡Ð}?6GûE·?;}šñ|	#?6GûEà?ïüÛájÁ?W;u	kü?9 ô¯ñù–?W;u	kø?ïï‡q¬)?aŠd
'?`xŽâSÖQ?aŠd
y?ïðè&Š³ã?M`ù¬9'4?^/²ê˜5þ?M`ù¬9'L4FGL J0001.5+2113?åy­éKÀDužèóÀ8^Äþ¢2À;Þ¿Â"O@O
"M@bœº¶IÔ?¡î[3?ÄRÆ6ɾ@L¦CÌ«@k˛ŸXJ¿Ï® yÈ¿äeßBp<ÿ¿èÀFA,ðú¿ìoN6ĸ+¿ïÿûÎBÓ?lÏÉëN¡AGNfsrq3FGL J0001.4+2120TXS 2358+209?ïôyàm£?`ºÄ՜l?W?É$»]?`ºÄ՜e?ïò%YØ̧?|DÔü"Õ?[µLNf±•?|DÔü"Ô?íè®Ý>Ú'?¢7Sr¿¢ ?°º‰	.Ì?¢7Sr¿¢ ?ïýí–>/Ø?'¶æäÓ?0"NAÙ?'¶æäú4FGL J0001.6-4156?Ö$L]…ÌÀRÓÃa@À:DOÀ1³×À<]yÞon@ —ÀÍe#?ú®oês¦Á?»xö"¼C?±ÛsÖôï?÷®·`,'@A=©-á:?í½¥|üªá¿ä«Kb©îQ¿ÑIò&ùi
¿ÑíñÀL5ä¿Ü}#Â'w¿Ïb9°ûµîAGNbcu3FGL J0002.2-41522MASS J00013275-4155252?ïþþXQ%‰?‡$©½R? zí§l‹?‡$©¼Ø?ïýˆ†tÚà?QvÅiÿ+™?3»ÌY)™?QvÅiÿ+?ïûsJo€?M®JЌ@h?B2ÖAÿږ?M®JЌ@_?ïö­Ë¡b[?Ay_<Çc?R¤h½;JK?Ay_<ÇY4FGL J0002.1-6728¿ãm5@ßîÀH{Râûã;À:'J7[·À<™øn;Fþ@ m#"'ÿ#?úؒ2>?Â	ˆ–.?Äõ¤îŒ@\	›Š4¢@Ï$'ҁî¿îèÌ!¬"2?Ï ¤Ð¯Z¿ÕºÀ°´¾¿ÔšÀ[¥B¿ÜÄ°ž˜Ý¿å«`"gAGNbcu3FGL J0002.0-6722SUMSS J000215-672653?ïî^#ú÷µ?]  óKúÒ?a¡ÜLè?]  óKúá?ïû‹èӀ-?\âíÀM8?AÐ\±ÿPË?\âíÀM.?ᅯ'þ¸Ñ?nÌñ£Ë#?€öQ˼?nÌñ£Ë$?ïÓVá´¨?cÁ«nFa5?vTõ%«ë?cÁ«nFa<4FGL J0002.3-0815?Þ:Æ$¸ÕÀPöK	éÎÀ;\tì;'À<¥S"'Û@ 'ev§Q=?þÚ ø2¬?Ñçq"Á?Ã7S=êœA?óM¹Nè›@ŽM¡sÙ¿ïÿú Âî'?ïþ–ÞÔ6N¿ÝüK€ª¿Úmïÿ
z<?ïú;/€÷AGNbcuWISEA J000236.06-081532.4?ïý݊*óT?0±©«!cí?1®¨eQž?0±©«!cò?ïéúŠ;e‹?'_QÙ?c¦?fuĚs—?'_QÙ?c¦?ïl®¢{ˆ?‹›3NWÓ?'j+°œŽú?‹›3NWÖ?ïØ÷£Bû'?p<'&o?s".^'m?p<'&r4FGL J0002.4-5156?ìéSЫÖàÀOÄþ'Q~xÀ;Á!\qÀ=dmgâg@ ÖKã*\?õ˜/6Np¦?áióïP…T?ä†Íyšö'?ÿuäô
ÿ8@/tæ±ÐG?êK7 ¦ê¿íƒgþìÛ¿èšð{þ~ ?ތ¦ æ{¿áL#ßÙ¿ïüò™åï´AGNbcuWISE J000229.20-515227.4?ïüíª%šC?;ðâw¤#1?8'®Ó-ð?;ðâw¤"ü?ïý¹ªLîò?FÑ
ÄÜ·'?22­˜ˆp
?FÑ
ÄÜ·"?ï¢%õƒ½Ø?†ª/Á»|?‡v'Ÿ‰Û?†ª/Á»|?ïú	Ë/Jr?E÷—?ÍØ?GØÓBÖ6Ä?E÷—?Íâ4FGL J0003.1-5248?¾3M7_(ÀOdüó0À:R"O…yQÀ<x|àü.º@ xŽÎ9‰d?üöYSXm?½°''¾?¬îþ%	yÑ?ó_6Ç<j?úжç2T¿éß5…
Ó¿ ©e>ž g¿áìáàZHK¿ÛY¶T»C¿ÑFÆbûLè¿äXY]ig£AGNbcu3FGL J0003.2-5246RBS 0006?ïùq'w[*?Cg‹p†×r?J9¶""Qè?Cg‹p†×…?ïí´Mjàñ?u¤µÕ­ë?bK²•3?u¤µÕ­ë?ïæ±媰?nùÞ²#ڏ?iNëUO ?nùÞ²#Ú~?ï™fô¿|Ý?w»H­"¤ê?‰¦BÐ Èú?w»H­"¤é4FGL J0003.2+2207¿«mäšÊÉÀC°½ãû½{À;0')ˆ†À<w2>@­o@iBªI•?è¢Ç
,¸?árh!ýU×?ïýt³è@1¬šþ¨?úMEââ¿ä;ËB^n¿í5K Â€¿èuˆb—7?Ð;œ£º.å¿ïfKÄ#°ß¿ïþ'"oAGNbll2MASX J00032450+2204559?ïÃð‰VwÕ?y9"ŸÓ?~»TÄô?y9"ŸÒ?ïic×ì?¯¬jgø›?'Óœœ%€?¯¬jgø›?íÛç3Š²7? d×&ë¾g?± ÆcªnR? d×&ë¾g?î͗'‰Ž"?¡ã|¢þS"?£&‡×gÁ?¡ã|¢þS"4FGL J0003.3-1928¿æؾ&<ÿÓÀS%.ßç[ÄÀ:‰HºƒôíÀ<w˜¢ù"¬@qŒž3‡@w°év?À½mÈ°?ϊ' U`@
D žq@œåGB	?ï¬ýw޿δ]?KDw¿â‡ôiÉÈ¿ä`‹[uN¿ë°SO2m;¿ïÿùJYQAGNbcuPKS 0000-197?ïIk"Hî?¯:þ$nLi?–ҍvâ?@?¯:þ$nLh?ïüן'[?V{êx'Š?9C{í+\?V{êx'Š?é<¸¨^?³Šž9íÆ?Ë
¡_ª†?³Šž9íÇ?ïꯕßqî?VWɶû¡^?ePj Ž¬?VWɶû¡X4FGL J0003.3-5905?ïåòhTnòÀL{¢£Y6À;Cü¯¨À<¼…Ñe¸Á@Ê\ñ*$@L€S?Á\¶î¿¿§~Š°¯?åýºËø<?øŸ5dæ´?ïíŠè%èMþraF¿åÉ3¿Â¿à8G¤Ú?|¿êwMt'I¿ïé\ AGNbcuPMN J0003-5905?ïõZÈpÁQ?RÛâ ñ÷?UJo}\7?RÛâ ñû?ïC!–bM?¦ÝÒY,?—›Î
3¶b?¦ÝÒY,?kº8Í?"àGŠ¸ëX?Šß%qÌv?"àGŠ¸ëU?îö"#Ù?ŽH–aØ9§? –'¾}Âs?ŽH–aØ9¦4FGL J0003.9-1149¿ï,Ä­·?
ÀQÄÎp:ûÀ:ՇΕú©À<¦[·¶»@³9Õs?þéÀùYó'?ÄNmRé²?Ñ[!¤?ã@
¾á77¥?÷çÔåõé?êªI¥Ò?ïЊA7õ¿Øarv?!~¿ãMDVq%Ý¿ãªèvv~â¿ïÿò"²¢AGNbll3FGL J0003.8-1151PMN J0004-1148?îÃh¹½þ?­v¿Pgº?¯sÉtd -?­v¿Pgº?æˆrxW"?Ô|=N†¶U?ÒïP×õ?Ô|=N†¶U?èr›,yÇ?¶7>Îü?Î5"Oúä?¶7>Îü?àµCZ?éh?¼9*$GV?ޕyK€-0?¼9*$GV4FGL J0004.0+0840¿ï€ž¤8šNÀJ2ìž#lÀ:ߍè‹o4À<&Žà4@aÖQZæ€?ú­Yº†y+?Òè‹o4kB?Þ×e,)ª@,œü$©-@oô0¿äõj¿'{¿ë÷]>Êk?«§½ý.È¿Ùý¥ýÖ.¿í¥è\uKÜ¿ä
NÒËêOAGNbll3FGL J0004.2+0843SDSS J000359.23+084138.1?ïÂG:æ%Ð?~	½ýK?~ÜbŒí²?~	½ýI?ïáÈÀõƒ?—f…ûT?n7û?
|?—f…ûR?ìJp~$"?ª~°ð"8k?½¬|ß»`?ª~°ð"8j?ïèdÅÝ=?'&ºŽ1?ž'ógDX‡?'&ºŽ14FGL J0004.3+4614?ÆÏkà·À/µ¶¡è´À:A´¶U'À<	*K-%@Hó{bKú@7<'W…ù?ÄRéF€?±:Ë^¸?ìt1ËT&É@m­3Tk<?é"€­ºc?Ò,&äñ0Ú¿æÓu}°"î¿æ6J²È¿ïÿÿ²}@¿ë
CQƜAGNfsrqMG4 J000421+4615?ïùW™%A?Mg°†ú£W?J£Á›jý?Mg°†ú£\?ïýùóLN?Iª@'½¯?00eŸ-4?Iª@'½¾?ï+G±ã5?'h²3M­?šŸ÷	Ùn?'h²3M´?ïñÚõMÏd?LrÀ'jxÌ?\Jda5É?LrÀ'jxØ4FGL J0004.4-4737¿ís?€RtÀPâk΅3±À9酿ÈŒÀ<ê$Ìh@G:ï•#¾@o-d½û?´Á«†?·»Il°'@-  ôØ@½Î°|µ¿Öš¢bë݉¿äà}ƒ¹^¿æwž™¿ã%ªê#õ©¿éˆÒ!Š_¿ïÿàU?ÍuAGNfsrq3FGL J0004.7-4740PKS 0002-478?ïþ~ :³Ê?!–\á×á?(üTÃn?!–\á×î?ïþŽÏ˜üb?@џÉ µ?'p9öo?@џÉ ³?ï×VÉEŒ?rďñ¾óÌ?tT›]9þ?rďñ¾óÁ?ïÿp\RZ]?"E´5·?ôu´´b"?"E´4å4FGL J0005.9+3824?﵆`ù؝À7¸dàÀ9œSÆP±ÉÀ<"Çȁ@p!G£X@j˜û(¸?¶Ã0òZ¦?ÈNÇ"é¹í@ô±î$5i@
LPóãg¿Ë&'¢È¿ânyZ^ñ'¿ê
ªB^Ia¿ëD§>ȽŸ¿êg <¶j¿ïÿüÉï£AGNfsrq3FGL J0006.4+3825S4 0003+38?ïó¨Ñ&Šx?^ºõ6òÛ_?X®]²ë1?^ºõ6òÛP?ïº2:"­>?•P˜ÁӐ‹?sq[°n?•P˜ÁӐ‹?îd,€~"?™'Ôs8ó$?©·í7øë?™'Ôs8ó#?ï-íéëæ?"­Y´
±Û?š_'Bƒ<?"­Y´
±Ü4FGL J0006.3-0620?êe¢@çìÀP¨òù‡@À;/#Dže/À<­\Ï
ï­@·-¶œ‰¹@ØTÛ#§¥?Í"ÆÔeH?ųNáåbÆ?õOl@!ð!慿ç0Ýî]@M¿·?ï.K—Ù¿ä'§
öbȿݶßz¤`ó¿è:Ë­èÛ÷¿É~-W|AGNbllPKS 0003-066?ïúI=é¤b?G	u`ƒ†?FÛYny«?G	u`ƒk?ïý÷ç	xá?MZ«™°?0@Ç´8ù?MZ«™»?ïº*‹&¸?'<g>Þ­?u|]6R?'<g>Þ«?ïù~L9ð?=p·XnÀ?JÏ=Îw?=p·XnÞ4FGL J0006.4+0135?ïôEÁœ«øÀM¦&þq‹À;'Æf>À<¨Ð©*0@t×#x€?ûÚЛŽf`?ÕaÂÍÅp?ԍŸ½~ü?ü
9‰Ž‰›?ý[ÛU{²~?é&>ÚH¶?Ž"Ñ,û-*¿Õ¹¼å#/Û¿ÝOõ`¿³_¿å¶³ «Ü'¿ïëñUBQ´AGNbll3FGL J0006.2+0135NVSS J000626+013611?ïíf"|ÛÁ?d¹Pz¤Z?b™{ƒ$A?d¹Pz¤X?ﲅo±Zr?šzŒ¢no?ƒ^¤©c¼?šzŒ¢nn?ïC²µ/Æ}?á¼óÔ?—‰©Z0?á¼óÔ?â~ñ/?'JÔ¿¯Z&?¦%1Øí?'JÔ¿¯Z'4FGL J0007.7+4008?å]×H8È«À5ùÙUmÀ:Ë
Tí˜À<fߥ¥@"Dˆ›¡?ÿ¿Å}M3?Ãß4®]uý?ÆøĤ•@á*¢jùs@	ýÛV}e1?ï6è)I¥e¿Ý'‡"-D¿ãœzõi¤	¿ØëÚcä+
¿êWAï8²¿æÞ+	Ë[AGNbcu3FGL J0007.9+4006NVSS J000741+400830?ïÝkÎêÞj?p²ú¸Y¬É?qJŠË#?p²ú¸Y¬È?ïú=Éý'ð?eBŸœg"Ù?GØ`B?eBŸœg"Õ?î§H‰ŠxÐ?œ­è™1,A?¥‹wgXs?œ­è™1,C?ﹸXòç?jÄhµïú?'ÿ)ÃF"?jÄhµïô4FGL J0008.0+4711¿ãQgÜSKZÀ..¥.ùÀ8¹¢‰à¿À;§=áâއ@ÞTû½?þÛ«©gm?¦%"¤DÃS?´A﹋Ò\@®jv–_R?ýÉ
mAL¿ßÚ£}ɿך/ ~û‰¿àŒ
ÑyÛ¿ÛsËßgD¿ãéoÐrs»¿æ3R3ÐèAGNbll3FGL J0008.0+4713MG4 J000800+4712?ï5¸~utL?•E~Ò¡ä«?™Hð1Qv•?•E~Ò¡ä«?ÙùœiY.?Ôɑ•·?ãw1ËSi?Ôɑ•·?ëý³2̉?¨o«5@~Â?À	34ÍÙÍ?¨o«5@~Ã?á8C—"´?³{ûŠ?ɕ?ݏxÐ÷ܗ?³{ûŠ?ɕ4FGL J0008.0-3937¿ïžÈ6'>©ÀR¥UGZ1¥À:½ÆßîÀ<xLuúX @Ñ"³U@+ã	O4?ͺš›!Y?Ú
‹t<è¿@»íx:¤@7Š:?îãË\4¿á롃rç¿éï¦`ÒRÉ¿ë:Ÿc2)¿î_ÌqæÍ¿ïý
':"AGNbcuPMN J0008-3945?ïg[+ƒÄ?•h?"Ÿz‡\?•h?îo*ʯu?¶b7]€Þ?©
S^%±?¶b7]€Þ?ìøG¥//?©)üLq¬?¿è=Âֆv?©)üLq¬?ì"àð?¨ØÉöQÛM?¿‹`ÿJ?¨ØÉöQÛM4FGL J0008.4-2339?ïÿÿà"LjÀSì6ŸÏ=ÀÀ:Èeü´%À<{¼Ñ­^@!"þäÌó¹?õ•ôäC?Ñm>Fâ"?ÑͅC÷%¼@xCx%@påÆBð¿ïîÎô©‹?ïùÑb]Ã*¿ÆJ>¨nڿǯ³ ÿ)¿¢/¿œsÏ¿éÍáõ¨äAGNbll3FGL J0008.6-2340RBS 0016?ïýÔ8u\?6]Dð?1^;|Ub?6]Dðç?ïû
—(s3?o':4Ëö®?CÕ£^35¼?o':4Ëö¯?ßö&3?‹$ã–n?Š'ˆvrÖ?‹$ã–j?ï.Cô?VêÊÉÍЯ?aICѼÁ?VêÊÉÍб4FGL J0008.4+1455?ã¤Rò@CÀGVžšÀ:J‹¤äPwÀ<fjbti^@¡Úõr?ÿÈ+}\L?ÃÖÅIُ?Ä|í'hr°@_&¼,k™@Ðÿ¿EÑ?ïñÁä;~[?ÀV5VNb¿ÛAÅݚOw¿àðž'ú¿ât"Ì¿ïÿÿ)@k*AGNbcu3FGL J0008.3+1456NVSS J000825+145635?ᅡ({Ò?|±êÇÉ2T?€uá:K©?|±êÇÉ2V?`¢2?šúIòÊÏ<?‰—'ÜsY?šúIòÊÏ=?ïó¼cÜA?"™e­4þ?ž!ˆs"w¥?"™e­4ÿ?í"
Oàl?˜¼DŽ_?³g­€üŸ¿?˜¼DŽ^4FGL J0009.1+0628¿æ+xYLÀKo$cŒ—SÀ9ö™"º]À<HßݵR@(É°7À·@*¢jùs?¶½'é("3?§_¾EdR?ñÇ=áâއ@Œ@ž'?鸞—@¿ÌGNž·Ì¿ãéˆà
ò1¿ß@?
Vñ¿á¨–¾•¿ßç¢ünÐîAGNbll3FGL J0009.1+0630TXS 0006+061?ïð_Mõ€?Y'xDû	?_AeÚ?Y'xDû?ïû'Yã'q?YRw-ºéõ?A¶˜sb6B?YRw-ºéú?ïÙó/k>³?x–ñÊ(ºþ?shJ`¦ø?x–ñÊ(»?ïÑK7aM?c!â³Ú'?wwZdOY?c!â³Úƒ4FGL J0009.3+5030¿ïÊMùtŽÀ'›oâæê…À8mKrÅzÀ;•L''Ù@»-݈ܳ?þ\Ü_? Ï¯Ù¡ò?¯ãçñkg­@§óþiýË@˜p=Ö?µ,ü€kö¿Ý€Á›ì/>¿ày`^dL¿Üdµ÷ž1¯¿ãL
Ìsá¿á¡ê€¼ÓÛAGNbll3FGL J0009.3+5030NVSS J000922+503028?ïþÙÓíH?5ÒÐ,1?"hÁ+zÛ?5ÒÐ,1"?ïùÄ`—´´?aøšjÞ¬ï?Hî}¡-,Ö?aøšjÞ¬ò?ïÊ! Š?\ær‰†¦?zï1oýºM?\ær‰†¤?ïùÅqr'ª?6ÿ4öM•?Hê:5¹Wh?6ÿ4öM¿4FGL J0009.7-3217?é3ëôñZÀSå¶ÃvöÀ;
Ë
Tí˜À<ÄFdh_e@I%Â1hX@¸¸]©ÿB?NjÑÅZÄ?Àq<XJï½?÷­_™Ã‹@л¸¨Rš¿ì)ˆ$&Oö?ïþ"4­†¶¿Þ5»8OÒ¦¿ç0ý~E€=¿Ùm"Ãqx¿ïÿ÷Âé±AGNrdg3FGL J0009.6-3211IC 1531?ïü»âö#;?:4‰.-G^?: èNæn?:4‰.-G?ïúþ*wG?`±³îAé9?DV"â¤?`±³îAé8?例šòȁ?ƒ"üæÎüÉ?†R™CMß]?ƒ"üæÎüÎ?ïîÙ&(W?Th~'ب"?a&Ù~ש
?Th~'ب¤4FGL J0009.8-4317?ßà‡É©Ó
ÀQñíåKIÀ:Ì{¥'Ì À<¿¹!]¹@¤ð'õJ@_¨†œg?¿ŠŠ2‰~?–ÃEÜÐrk?Ù|xl·c@¡d½Cî?ïý7˜ól¿ãGêüó¿àeê«%)¿ãŒÿÂÃ^¿ÊËîÖaöë¿ïünEWøåAGNbllSUMSS J000949-431654?ïþ¥¸Z3Ó?$Æï~¸â›?%¤z\ÂÞ¹?$Æï~¸â:?ïþgn‰/?D*"ü§½?)‰n}!¯?D*"ü§Ä?ïë"9"Ø(?m¥
ý–QT?d{Æk'×5?m¥
ý–QY?ïý•¼
VÆ?%B¥6/±?3R•IÒ%?%B¥6/y4FGL J0009.8+1340?â쀉¯gÀGüU\Rç.À;W
F9 5À<Ÿ"Ì'úò@5 t-Þ?ÿ1-=¾§?ÝI–a€Îr?Ìô@ÚÖ?ñDœ¸2@ý³Š²K?ïâu@ýA¿ë¢&Á	õø¿â¦2ƒ
¿×Ï`ۍ
¿æÊf¿ïþ^	 '²AGNbcuRX J0009.9+1341?ïüÿ'-'i?9{±+…%4?8v–ĶX?9{±+…%"?ïøˬ¡¤?bŠlQªG?LÑMyoªâ?bŠlQªH?ï§`%DÙ¼?‡PÀv"o?†'ö®ÉÀ?‡PÀv"o'?ïàb°iñ˜?]êï±u?oO–g€?]êï±{4FGL J0010.6+2043¿îæQ¶÷KNÀDk&¿‡jÀ:àÛŽ,~À<W÷7Ú@ïùR¼»]@þÜ~ñw§?Ê9R‡w'?µ|Û·Ì5?éðüVþ—@
ZɈ'?ïÌöˆ‡ù^¿à‰Éb4'¥¿æ8a¦
Ec¿äyïøK¿ïý÷è‰ø?ïå Jù"–AGNfsrqTXS 0007+205?ïÿ‰I
z†?
2Øà'?
­½a^v7?
2Øà'Î?ïýÉû|7ó?GˆIU\Ā?1°$@nñ?GˆIU\Äq?ïÏzú')6?xp(bto?xB'¶ëe?xp(btg?ïûÏä)ðH?3¼Ê_†¹3?@ÀoX>ãƒ?3¼Ê_†¹4FGL J0010.6-3025¿åbaÊ?ËÀTÞ?»×²À:-úNwÀ<‹3b-Â@g@õ¼@$
COàé?·Œ~Óð'Š?»)Üâ‹S@R'IðäÚ@Éh>WÔ?é¡ªñA¿âLý|íç¿å9ΛÙæ¿ë÷…¿â¨°"rпïÿ÷fÔJpAGNfsrqPKS 0008-307?ïÿo¥òD¬?Þ>xðq?A·j™Î?Þ>xïõ?ïþ8)Lb?J efrù†?.¬}k9ãz?J efrùs?ïßwĸÓP?nèÁLJ×6?pD£–X±?nèÁLJ×5?ïÿÿJuÂ?ëïŠX?@±G©†?ëïŠ4FGL J0010.8-2154¿ê'ß:…!ÀSÙ¡ß¹8›À;3ö Û­:À<»:{&@jˆûf¾%@nLa…V?ÃÍzFÃý¿«H^éop?æGߒ¢."@ž¥]òú^?ï߂ˬç¿Þšù*3°¿æý¾Ý ¿äƒž?ò¿à¥R©®e¿ãûxFbºàAGNbcuPKS 0008-222?ïû%>iú?@¢_§*£…?CkXŒJ?@¢_§*£y?ïûD˜ÌŒê?_Øد¥G=?BíœÍÌUÇ?_Øد¥G>?ïÑÚ+?w!¹Ž+?wôê~_?w!¹Ž%?ïù®ã\ƒc?:ÎIªž5?IDròn?:ÎIªž'4FGL J0011.4-4110¿äDٍՠYÀRn!ÄuæÀ;D°P$ÜÀ<³@ý R@v^í T^@(z§f?ÐѦü-¸u?ÄCcW`€?ðö›r¸?ù©«?^dº?ç"0ý
'¿ç§0@9«ó¿éPÁ^.´s¿ä¾cþW3n¿ïý
ýn«.?äógkI$AGNbcuPMN J0011-4105?ïäÓ¾É?p~ü
©k ?kr,A6å?p~ü
©kš?ïmiO0›C?£,ºX	?'RÖ엪?£,ºX	?îñ‹Bƒ?–S/õc? çKÞ÷ç?–S/õ_?ïTÍo½?ˆ~Ak'+ü?•}pR_?ˆ~Ak'+ú4FGL J0011.4+0057¿Ó?dÌ}#ÀN&¾œˆacÀ9ô–Å©ÂÝÀ<N­\Äüõ@L€oüè@IHÜä.?»ÞÿÝp^?¨:g³?êþ;¹ÿk@ö5¦Õí¿Ýù¥ÞÍ«¿å溌¤¿¿å×w¶á¿Û(RšǦ¿ëøV¿ïÿójÆGxAGNfsrq2FGL J0011.3+0054RX J0011.5+0058?ïý‡6‰¦À?:í[²?3ÆK²Ê6?:í[²9?ïþÙ'W?LW.—U²?.òmŠ³Ý?LW.—U±?ïÙhÿ»Ö?w4îô*?swK€"_?w4îô-?ïÿMP·jÞ?
âëUç?Ué¤?
âëU 4FGL J0011.8-3142¿ê¶—<	 ñÀTõƒ¥À;N²™DàÀ<ÓNáåbÆ@ 9ûIaó»?þ²ÜæöC¿?Ì]TS:?±]íÆídÈ?å>lý"O°@…'¤Ø'?Ú%â]ã°¿ëÚúWI'ñ¿â€
¡©2"¿ÔÞ¤»Œ¿Úyb&ñ†¿âd?Ÿþ¶AGNbcuSUMSS J001141-314220?ïÿ©ó³·>ý
Ç~Žá?ƒ9Óì@>ý
Ç~¹?ïþÎkÈûC?<e4²r3T?#CpKÍI?<e4²r3T?ïûÑ;×10?O‰5|+x¢?@»£;FI?O‰5|+x¶?ïÿΜJ6?¹2²ÍyK?,v¹pd?¹2²Íy[4FGL J0012.0+7043?V,è@ 9(| À:Q/|À;Á2š†ÿc@
žÇ2@=v?ø="?¾Ñ8Ñ¦Ñ?Š›ÓRt¾?Ïý"ÀÁќ@tâÕø›?ï^0§g¸¿ç
µÂÅ¿ç
ˆ~¿¿ä'1}Ñg¿áEÅÜïüÆ$<kAGNbcu3FGL J0012.4+7040TXS 0008+704?ïñ±C•?WòÃøä?\œäåx×?WòÃøì?ïûÿih·?c>ÄSîý?C"Z] ¥?c>ÄSîý?ï¯Í‡®ä?ƒÖ-˜|ö?"ž;F™?ƒÖ-˜|ø?ïßaþÓA1?Yf º˜™"?pO–_f¡?Yf º˜™‹4FGL J0013.1-3955?éfTÀR»ê šª;À:¼b~À<vA
çI@½PdÇTé?þ¯¼†-¬?¸|)ò?½€{:ˆçñ@æ"FsØ@øv3xR¿îÄ"YFB?ÜR–»B᧿ཨ6ëN˜¿ßɯvz° ¿Ü¢‰'JG¢¿ïáGãÄ`AGNbll3FGL J0013.2-3954PKS 0010-401?ïë"
Íè?k3ª'×ÃÏ?dókõ2Ì?k3ª'×ÃÔ?ïä"îÁXo?'µÉ<-?kk>§'?'µÉ<-?ï9R%j?'Ø~Þr?˜Õ»R¿!?'Ø~Þp?lævÔ?{);õ:J?ŠÓäÆbJ¾?{);õ:I4FGL J0013.4+0950?妈vÂIóÀIóƒ@'À‡À:þ¨ø².À<Y·ø)qé@ (ÇÉ@ёW«¹?ÂGÞ;	@q¿±6"K~®‡?ççÛFSË@¼ë-`
'¿æt~7¸~¿éGúÀ{ٿ♅CÛ!¿Õ!â"o¿å®‹cuñ¿È2G%˜âAGNbcu1RXS J001328.4+094942?ïü!/€²?8æ͜ßø?>÷^ƒúh?8æ͜à?ïýwˍ?SŒ^ߖ²3?7ÔG™£'Y?SŒ^ߖ²1?ïå-®á	w?zJóp"ÃX?jÒQö‰~?zJóp"ÃL?ïùG'ŽK?=ÌTi-n2?JãÓaÆЂ?=ÌTi-n*4FGL J0013.6+4051¿áËsE½&>À5svæj±À;ªáÀyØÀ<ž&~ïÊ@â¦J,@ÓjZç­#?Àz•ÈSÁ¿ª4
x¹z5?êE&z¾@@Û+'9֐¿ê ÛýÂ8¿Ð_f,"ÃI¿å¯wè]L¿âF(mÝS-¿ëyð¼–ä?ßú1Ÿ_VRAGNagn4C +40.01?ïÝ'"TæÄ?p‡¡dmë–?qlnՌ»?p‡¡dmë•?ïû#/0™?b˜õ<ÄÌ{?CsCŸ=šI?b˜õ<Ä̀?ïw{8>Qì?Œ¥kÎ-6p?'˜ø5Â[?Œ¥kÎ-6m?ïð"Qû®t?P}üŒ™?_»\£_?P}üŒ™¤4FGL J0013.6-0424?䝠˃¥ÀPcgM3HÀ:îÍ´SYCÀ<9òYNP@gzÃ?°D@Zþ¾·`T?Ԉx47¿±ÆÆ£gùŽ?ì´Ê(,o@r! 
Ò¿ì?"ÿ%åm¿ãm•ßû¨­¿êÑà2_¿ÛÄBÚÆ	º¿Ù›pß;9g¿ïÿÿÊPËAGNfsrqPKS 0011-046?ïù£LÆïz?I§ÿigMK?IrÌäB?I§ÿigM-?ïøgþ¨?f,¸¿æ?N`]‹ ý?f,¸¿æ?ï͸}š‹•?x[Hqn·?y#Á2º5?x[Hqn©?ïøu#'I?@ewHtV?N+sbÛ»
?@ewHt]4FGL J0013.9-1854?æ
ꇅ[ÀS…âlvKÀ:m» ÒÞ_À<…©²'b@K¶¤l[?ÿH‹¤äPw?¾`»ô?£Yÿ$ãº?æQSåZbL?÷¦è\JX¿¿êÝ´±M†¿Ã ÝE?û¿Ýc-˜pû¿ÝdŸý5ö1¿á—¬ÂkJ¿ÜFàd.RÏAGNbll3FGL J0013.9-1853RBS 0030?ï÷e|¨?I"ãxi¾þ?Q5ËÚ¬j?I"ãxi¾ß?ïÙ'Æød?ˆûõ?sulƒÍ]?ˆûö?ïٚyb?wàž46Dè?s2ÃvN±?wàž46DÖ?ï ç9D"?vF
(Á±?‡Æ1®ú[:?vF
(Á³4FGL J0014.1+1910¿ãÙØ1YJÀEiÕ^kÆ"À:¤z
ˆ?À<ƒ€!ùO@ Y:ƒßs@<t$•?ÈùùUÁÓu?ÉD‹ÑYú@—Oµò–@
{I.óŸ¿Í-÷I£4¿ÜÔì@…4¿ãŒ'Á)i¿âñ¡§Úû¿íÇçÀn¹¿ïøðiŠAGNbll2FGL J0013.8+1907MG3 J001356+1910?ïæØsֈ9?iìS¶æ"…?i'Œ)wÇx?iìS¶æ"ˆ?ïýÔ¨hãr?N5Š–Éì?1Z¼¸äk2?N5Š–Éõ?°"@ê?–ìNô˜ÃP?¥§¤öËñi?–ìNô˜ÃT?ïô#Ÿ?H'ÿ'Ò1«?W¹ÝÌÞÀÏ?H'ÿ'Ò1¸4FGL J0014.1-5022¿ï¡rD<'vÀPlwÄ\»ÃÀ:"TýˆV{À<»à'ó@ŠÏ«úDT?ÿ{7(‹9…?Á
!«¡"?¡7öx±?àj|«LI…?ç¸øaœæ?ï(þûž¿éˆ—~6fÄ¿Ù#Ìhù¿¿áÝßÊÖS¿àg"Ý—ö+¿àp¯*$–¸AGNbll3FGL J0014.0-5025RBS 0032?ïúÉY<?HãÁW5r?Dڛç
Äê?HãÁW5a?ï0Ÿlã'q?¥GK•\6?™ìc›Â?¥GK•\6?ïÙ½Fu;/?w+¸ÉJ?s!\Åbhh?w+¸ÉR?ìåæ1ªWó?¢ú¯}
É`?¸ÐÎr­@]?¢ú¯}
É`4FGL J0014.2+0854?æ1'³ŽK.ÀJm²•éâÀ:ÆL²`9üÀ<$ü.º'¯@p.#(ùô@á~4¹E?ÄBáÑ윿¢ÀÛkT?Û¬ƒå@ýTƒ™¿ï9¡v\Ô?ïùƒyœ¤¿åñ™ O–@¿ã.IW¿ïÿùŸé"Ú?ïÿ·ÀÌ
ŠAGNbllMS 0011.7+0837?ïéTÝr¥?iž]ò´ã?f«"Zâ?iž]ò´ã?ïÛÚyù‹@?Š$´†b±?rÃ:`?Š$´†b­?î²þ…Ѹ?˜é‰ûÌ°?¤Ð7¢äo?˜é‰û̱?ïÛ-!?m6.w[J'?rwi|ovß?m6.w[Jƒ4FGL J0014.3-0500?àµ{,IÀP‹¬GG"À9þ!e«U"À;ó×Ûô‡ý@ÜÀ? ©Ù@Öæþ¸?¾á@øÔ2?¢hEÿ/Ý?äÓìŸ@ÀëNB-L?ë'm{-È¿ÚíÎm¿è¬l°{¿Ü;ŽK‡½Ï¿åÆ û;¿ðAGNbcu3FGL J0014.3-0455GALEXASC J001420.46-045929.1?ïú¸ªŒ&?CU€m®u?G©UÏcy?CU€m®Œ?ïýÒÓëô'?Gm¦cÆ¢"?1i` [r?Gm¦cÆ¢?ï´|6äŸ?ƒPÁ@[þº?'àú2F؀?ƒPÁ@[þµ?ïî¬ÄJr—?OøOzâô?aS;µii?OøOzâø4FGL J0014.7+5801?ÐÃr5iÀþ¡]³9À:ŒäxºüÁÀ<Uò#žjº@"R·Áø³[?øÙ<|ˆÛ?Åå¥vF®:?Ɖ·ú,×O@A&PÍ@‰¡a¿ïá@Âgîý?ïê'ñ¶'!¿Ó~°_-âç?­Ì8þ#[û¿ÔÜX[
葿ߥ83M4AGNbll3FGL J0014.7+58021RXS J001442.2+580201?ïøZ#¼y?Mè/l¹z?OΗq¡?Mè/l¹}?ïïR¥÷þÒ?If´¹K‡?`­Z-<?If´¹K‡?ïÇñˆÈP?~E´–[¬?|;÷›Ù?~E´–[³?ïÉÙ¨Ò?lÚ]t¸£?{q+ô–}?lÚ]t¸£4FGL J0014.8+6118?åÁo'?Ä¿ôr6~ANÀ9u?èM[ÓÀ;×4ÊâçÁ@ Œ€¨ô?þjbßÉ(Ó?»M•ŸŽü?ÁëvÛÿo·@líԄQ3?ý
ÀN\¯¿ëgT7¹F¿¤^ÞMu¿ã¬Øpnýå¿Ùìý™É?¿ÞRe]Qꮿè
þEjÃAGNbcu3FGL J0014.6+61194C +60.01?ïc™+\Ù?‹!Þ¾ü?ŒÚ"d¿?‹!Þ¾û?ã[ÇwàiÂ?Õ³¦z|?ÙHq?,|?Õ³¦z|?íÆtDÞ?£Á¶ØË>?±ÏL]ß?£Á¶ØË>?çÏ¥ÔÇq?µð!"zÇ?ÑÜ`´Vq?µð!"zÇ4FGL J0014.9+3212?ã"Mäq6À>™»'ˆÛÀ9ض쐷sÀ<^xîÿ&¼@a]Uñy*@}_~ë˜j?¶'+èç	º?Áú
ø' Ï@5µœ.ŸP@¶`˜Ëþ?xî(g¿â–NöÞO¿é¦'™ð×n¿è€åM¸¿ï÷™)1Q²?ï]€C‡>MAGNbcu3C 6?ïüi&J%?<æ:š¥.H?<·žÍ®Í?<æ:š¥.Y?ïù6"\"?h|Û.—{?Kç%ž?h|Û.—z?ï²5ÕB¸À?nƒßqžÿ?ƒrŠ¯QÏÓ?nƒßqžñ?ïêÄJ«ù?V¨äÀƘ?e;µTîÝ?V¨äÀƔ4FGL J0015.2+3537¿©£·­£Ý.À:­qGÏ¢À;x–z*h‰À<Í@N¤©@!8ÞZh×/?ÿKùƒ<Ú?į	Bsí㿤ä¯þœ
ù?âAªŸ¦N@¾ÌY	‡¿¦XåIpag?§‰\¾$›ô¿é§h5"¿ß¼MΕ¿Óz۞ ç׿Ö±MëE^AGNbllRX J0015.4+3536?ïùDàHý?E«]¬6B?JïÜ~Ü®?E«]¬6f?ïý4W…í?Pˆ
=¼?3ö]CГ?Pˆ
=¸?ïëÖی¬?oè
£:Æe?dù)$sS¶?oè
£:ÆM?ïêMŒù‹ƒ?UªŸîŽIA?e²st{è?UªŸîŽI>4FGL J0015.6+5551?´(¾¼À Õ}uv¥À:-ñŽM5=À<@â
K³]@!K'Z°Ð˜?þxòZ%?¹7ʜ›×Œ¿p÷B"ÓÈ?¶6)Ôº­@´€Ǒ?ïþrÎ\¿Ú),VJ¿âôÿý²H¿ÚP*¥Em¿Ûšëÿ!Û¿Ò£'™¾-AGNbll3FGL J0015.7+5552GB6 J0015+5551?ïûg¹ìû%?Aˆf1?BaLpÊ?Aˆf0ú?ïýo¡Ï\?S¡/¶Uîb?4'ñ‡ F?S¡/¶Uîj?ïÙ@8b?«?zꫪ5Æ?s_ãÎà*È?zꫪ5Õ?ïÒ! ?aûDgªõ?vðo{õ°;?aûDgªö4FGL J0015.9+2440?î=A»VoÀB¾µ²ÔÔÀ:Ñó¹À<~µI"ˆÁ@ã&T'Ÿ@ç!éB?¸@ï3t¿±¯Vš@ˆ†?ù'KiŠÞ@ºÄNÎð¿ã|VÝÝ@b¿èÄ(Lýà¿æ	¢–"¿Ú0±CŠÏ¿æÕu³
ƒè¿Í¦ÙÉ	žºAGNbllGB6 J0016+2440?ïüòVy^_?8á‡<{Ò×?8mL5
?8á‡<{Òê?ïý¸4û?Lä]¡áP7?7j>X#~W?Lä]¡áP2?ïæ¸w5]?x	ô‡zõ?iGˆÊ¢åú?x	ô‡zç?ïòíÌd«Ä?IçEÓE†A?Z$g6¨v¹?IçEÓE†24FGL J0016.2-0016¿î+ЬäÀNí$ò'Ð)À9oßÏpÀ<&4ú³å@­ã'K°@èƅŠîÜ?³{qæLOº?ǨƒÂAÙi@€8AíH@¢,**uõ?»\$š¿	¿åÿ$£Mw'¿èç6oþ•¿î´w JŽ¿àŠB
ÁŠ¿ï¼=Ó %¥AGNfsrq3FGL J0016.3-0013S3 0013-00?ïýÃȔ‹+?=¡ØþùJ2?1á»[¦£9?=¡ØþùJ1?ïð™æñJ4?—@Œ²Ÿ?^Ì2k"Ñ?—@Œ²Ÿ?îo¤`Kž?œáæûtëÿ?©å¹ûF+?œáæûtëý?ïí§¯­õ?WtÂݤÍÄ?bXPR
öv?WtÂݤÍÌ4FGL J0016.5+1702¿Úª7h7 CÀFƒÑ¼râÀ:³dÀsøöÀ<j³fÊ9@0ù¼‡°@€ºˆ&«?Òç@ìY?Ó¡$'|œ@Ö_Æ	@[Õì¿æžï!‹k¿ä±^ýfr¦¿äì['û¿ëÇ4<G®ë¿ïÿ!Ÿ>õ?ï÷ZtÀœ=AGNfsrq3FGL J0016.5+1713GB6 J0015+1700?ïü¸ðĖT?B·çXF£O?:8yÛMe)?B·çXF£T?ïéuõû¿D?¼¨Y"?fŠ
@½0?¼¨Y"?îÛÔ9β?–û:@×?¢B¾<cï?–û:@×?ïâù–øµË?cÀÃ÷?miJ5E?cÀÃ4FGL J0017.0-0649?ÞÅÄ(X)ÀQÙŽuyÀ:_ŠªŽÀ<`íjÒò@"†qsµ¯@9^Æ^ô'?·]HZŒ¾j?ŸÐ‡†5}?ægf
öÔ@
63ÍÔ?ïʇ½ùö&¿á#W¾,öÙ¿æ	8æ0¿àéT "¿ç6
]ÑíH¿ÛcS!DAAGNbcu3FGL J0017.2-0643PMN J0017-0650?ïûõ'~Õ?:ŒÿAÄ:?@)÷⨽?:ŒÿAÄ?ïþB̾m?KUÉsž—?+Ó>¤6?KUÉsž´?ïí×]Ó?pÛÆ
`E?bbà(¢,é?pÛÆ
`D?ïú²êÊe?7ƒýÒ­oÐ?Gå4TÖk?7ƒýÒ­oá4FGL J0017.5-0514?èç˜càåÀPª½Qï·À97@´%6À;ۀ
×Y@㵈b—@ÀÓ¢±p?­xm'—ýì?ºé'9Xç@	HdóŸŸ@ÁI©lJ?Ð]÷ÂnÏì¿äŠ&ßè³]¿è-©¼&Œ\¿ér*ŸÔy¿ár\=îx¿ïÿþó…õAGNFSRQ3FGL J0017.6-0512PMN J0017-0512?ïÿ|a?ي®úæÿ?Ð~óÞÍ?ي®úçñ?ïý
Ò]Ž¦?Q–Uë ®!?7©mŠÊË?Q–Uë ®/?ï¤Xt˜ž?ƒ€Ý•²õÓ?†éþâÙØÌ?ƒ€Ý•²õÖ?ïþç±?¾"byÀ˜?'.a…
‰?¾"byÁ34FGL J0017.8+1455¿áZ3‡: ÀG•{t¤ÓÀ:£ß\òI^À<‰f1A@s~"?jN@?L¤?Í_,
u?É$Bjۗ?ûqG6w@<¼K <v?ïý?ѧ¿ã/+f¶¿à("` Ò¿àøý!©H
¿æ6""Ý¿è­-]AGNbllGB6 J0017+1450?ïñµ³[I"?_D®Öîè'?\"™Il×Ö?_D®Öîè'?ïû‹:íºH?]±Û¯.
í?AÓIã??]±Û¯.
ô?ï"œRòÛ?ˆ
ƒ‰äK=?‹8ØëCHË?ˆ
ƒ‰äK=?ïǵÃm%%?dKÍ:¥ë?|%Immq?dKÍ:¥ì4FGL J0018.4+2946?ÌÍfŸ»ÉØÀ@F-¶°`À:[ŒõFhšÀ<RùôMDV@!JË
)úz?ù€ÝàñG?Á*Á_0g&?ºäeb…[?ü}w$#Ë·?ùjž"dÿ?ïx³ÀŒLª¿çHº•"<¿Äê0_ï(í¿ÐQõ–²Y¿álîu"Ó?°m®^kAGNbll3FGL J0018.4+2947RBS 0042?ïú»Ý¯'??´#K€gØ?E‹ÑCfx??´#K€g±?ïµ»¥.½?›ÄjËË?'¾Q´P"?›ÄjËÌ?ïÜ"ҁÀÏ?vxìIÖ?q˜}?vxìIÝ?îfáLóV?'·0ÞLV¸?©'ë0ʘ)?'·0ÞLV¸4FGL J0019.2-5640¿çÇ>­ßœÛÀMòÜ­¡À:m'§7À<³[bý%Z@C+xÕ@_±%§Yv?º ZmO?¤-7#`_ð?éÔò5<!ï@O•¿ol¿ÂסçñÁ¿Ó§ŸÁ¦Óê¿åܟ]}ß¿ÜPLßÖë¿ç/§Ã(]¿ï¸uý³¦AGNbcu3FGL J0019.1-5645PMN J0019-5641?ïÿ¸^xm?
æGÚ¥?hô0ò^7?
æGÚ^?ïþ±Ãsgš?B²¡HQËí?$ãÈɆfÞ?B²¡HQËó?ïçÐÛFÚ?pîD"m?h/á$¹%¹?pîD"m?ïÿÃÆ
áÅ>ó[š
.ì>þùÌ5>ó[š
0Œ4FGL J0019.3-8152¿í7™VÌÞ ÀA"¿]xÀ9µo`
+ÓÀ<IîsÂ@N1‰9úù@šbÞòi?³f"nd6¶?¥B<Ä	7?ò@‰ƒœ@½×¿â úa§°¿â%\°Úÿ¿á}Gô‹W·¿à\øɪÙ]¿à×~0‡‡¿èï;!>>)AGNbll3FGL J0018.9-8152PMN J0019-8152?ïü»|žƒ5?4¬	èª.Ö?:$æS?4¬	èª.ð?ïý/^\…ï?RRÄñl!?6…
Ð|?RRÄñl!?ïô™ãþ?d­¼ªîð?WàÌ9î™?d­¼ªîö?ï÷hƒ?R
³~äÐ?aHo—|(?R
³~äÔ4FGL J0019.6+7327?Ô
zíµñ†@%sõ/ÂekÀ8¬ÿ˜Ñó}À;cgž@–×í<X÷@ÛVà·e\?¬¶áAèœ{?²ûðü¬äO@Å6B²,8@DVÇ?ïÅÒr(;ˆ¿á
/þËLš¿é1rEî¿äõ¹?§4ã¿ï¨ÿ"_{f¿ïÙzé¯AGNfsrqS5 0016+73?ïð=°Ýđ?be-šÇ®?_"žDvßv?be-šÇ°?ïös`ç‰?mGzzZ»é?S>1ÊñL?mGzzZ»ð?îÎDÝÁoä?–`RíïÕ
?£²#éµ?–`RíïÕ?ïúüb"?7¦LÏØd?Du¯¯ù?7¦LÏØP4FGL J0019.6+2022?ïbSß^DYÀDð\|ؙÀ:Z°,ƒÊÀ<|à"&þ@»½•LWò@è"ÿ‰;?¿Ì[㫌?¾[Ó µ'?ü§›4¤L{@*Ò2<h;?ïýròe㊿¥}¯-T¡î¿âë}'üf¿ãٔü{ç¿éì×.OŸ¿Ôܐ¤¨koAGNbll3FGL J0019.4+2021PKS 0017+200?ïæýˆPûâ?rðX*š?iw¯w?rðX*š?ïõ£Dî£r?mbߗ2GF?T¹v"¹º?mbߗ2GE?ïRåøpÌ?';ž\ã•Æ?•£]ñæg?';ž\ã•Å?ïãt"Ñ'?v)ž
«}"?Œ‡"Ú˶&?v)ž
«}%4FGL J0020.3+6919?æRÄ}[é@·¿ŽaÀ:>TÁù44À;£©8s@ºy³ +@ËYÝÁç–?̳*yÑ'O?ÈOÊB®Ñ9?ýóÂî?ãË(²H3˜?ï;ØÞ¨íJ¿ÈʺÂH¿ã¬Y?6vµ¿éZoíÎ¥¿ïÿú¡œGt?î  ¿'ȜAGNbcuTXS 0016+691?í\y&®÷?Á9êñp?µ6ʏ`F?Á9êñp?âr_ì8é³?ØQiêÞ¸ª?Û@'Ž,™?ØQiêÞ¸ª?åfÊ0p9?·+‹Š?Ôå2kŸŒ?·+‹‹?¾Ý'Ix¸å?«6½böú'?ì$MÖÐèä?«6½böú'4FGL J0021.0+0322?ÂÜɾî2óÀMOÀãŠ~tÀ; a3÷~À<™A<á1ß@ »ÚҞóÌ?û6ìü=?ÐMØ%–¯?€Å'pÛ?õ<¸gºú<@éä.b?àI '–ó¢¿â!3E¨¿äp¹pÏuô¿Ïp-åk*¿Úaj~#Ž¿æ`–
õAGNbcu3FGL J0020.9+03232MASS J00205023+0323578?ïÿ?KKðv?}æNvÝ?–ñn"?}æNwQ?ïþl—Þr?FlïÞŤ?)6'ßèï?FlïÞŦ?ïö'd3X?`Õµff¢¹?S±7™ÝPl?`Õµff¢Â?ïû'ôÎ9?3Y£ÓY'?A÷¨,Ç?3Y£ÓYº4FGL J0021.5-2552¿ÝÜ*¹;ÞÀTÌǎŸj"À9¤GOIê/À<WëÃ¹ÿ@¯mŒöH@§¦tso?°/R¾hÛâ?§ùâ&Â?÷$êµë߸@#8Vˆ¢Ñ¿ÞgÃ}î˜O¿ÛyáBz£à¿á$ý°šg¿àl°Ý­ð"¿è=[‹`œ¿ÔÄh¥/úÅAGNbll3FGL J0021.6-2553CRATES J002132.55-255049.3?ïú9³?DŠt}@?G‹Í3Ì?DŠt}E?ïý¨6®'û?P?râ L5?2¾JŽÀ*Ÿ?P?râ LH?ïÛgi[©–?vóY®¬k»?rLKR+4ä?vóY®¬k²?ïú¸S@;?9µn?Eº²ÿ}?9µn+4FGL J0021.6-0855?&óçöÀQžc^J8À:÷ØcÙÄ,À<Ÿ#vý_@Ñ£žU@@DXÍ?Ô5lÉV÷?У–r¬?ûü'¶vI2@£&T'Ÿ?åð ±»ÏO¿áv+ÀÎð¿àvÔb˜P™¿æ.Å_ñ_¿ïÿþÐñ¿îkV斢AGNbllNVSS J002142-090044?ïÖ»*hü¢?uuÛb¨²­?t¢jˁ¯N?uuÛb¨²®?ïǏ@â¢@?"L˜å½±?|8_Ž®à†?"L˜å½±	?íº7,TÙ?ž"Ò:lÒ?².FY7?ž"Ò:lÒ?ïR\àÂa)?ƒBÝÍÀ¢Ž?•´cç³ÚÅ?ƒBÝÍÀ¢Ž4FGL J0021.9-5140?ì³DS9nÞÀP5w ÈÍdÀ9¼•*™1À<i㤦©@ž4E,@m^•—?°F¸ Bj´?ƒ—»W¦Ò?Ñ}0'S×Ã@cː6Äb¿Ætž7ŽÇ¿äÑå©és¿ÞaOÛàf¿àLJžDy,¿Þá\ü°?M¿áñŸ,ݯAGNbll3FGL J0022.1-51411RXS J002159.2-514028?ïýÿ=R?%€‰ç\¤?0†…n?%€‰ç\«?ïþг´[­?=¨"*ñ'_?"ôĺE+
?=¨"*ñ'a?ïõC¥õÅâ?dܶqõÛ~?Ux´t=Ç?dܶqõے?ïþÙjÓÖ?7±¤
C?"iRžÕ?7±¤
«4FGL J0022.0+0006?íÒ»TAæÀNí؃º4DÀ;/…(ÉÀ<~CvwU¢@#zISž?ù;ë2éaX?À2AƞàU¿®p——¶Àq?ï"{[>@×ä"Sçß¿ï&%z
?ïþC¢|l¿äVÇ¡Р¿ãȑ¿/«>¿à@óæJ?àâÙ,,¯AGNbllRX J0022.0+0006?ïþ²xÚ¢?${ Ì†àÀ?$Ö(rUØ?${ Ì†á?ïóŒ¡ùÄE?x…áT8?Xæ¼ww¸?x…áT8?ïÝïäLG?r¿¦N:¶?q
òÙܛ?r¿¦N:¶?ïØy,a×?p̀py_½?sÃiÏr'?p̀py_¾4FGL J0022.1-1854?íuU¼KϑÀS×õY³Ð}À9Ÿ‡mG+8À<æ¾æZ=@2ý2Ys?üI(gþ?´Y¢ž%•?ºë¬ "ÚÆ@¼uf´iÿ@#¤^º?î÷*¾ðk8¿Ýµ‡9᣿ևî@¿ØM´ÿ%ºz¿ç‹^Öw¿Òl"h	ԕAGNbll3FGL J0022.1-18551RXS J002209.2-185333?ïøy
ý?M@'•âÖ?N×Ü¿ò?M@'•âÜ?ïҞ»i™?¥-á¢ÙŽ'?v°¢Kp4Ž?¥-á¢ÙŽ'?ï½'fúŒo?ƒ£qï—L?€¶&A\ä?ƒ£qï—A?女h\òÿ?uÂ
f¦bˆ?†_¥èÃ@Y?uÂ
f¦b†4FGL J0022.5+0608¿ïòü³GʺÀLl
oTLÀ8Ÿ6}jŽêÀ;¢OYÚg@û£è§ô¦@|\qðÞ?¤ "ˆÞ`s?ªMúY
°@8ÑØ¥H@F_Á܃ϿÃGw£O¥Û¿Ý¸¼yBŒ¿ã7õfI
¿á0[è^"Ë¿ã–#£Â¿ê
©ÂÉnAGNbll3FGL J0022.5+0608PKS 0019+058?ïýŒr7»?0S@¯-m\?3ŸìnB*6?0S@¯-mS?ïüq"hÛÂ?Ux%•ç?<vì¹!ä?Ux%•ç?ïˆM©Y?}Ç)•?z<ùÙ+RÜ?}Ç)•?ï÷†›îu?A82³ÚÅË?PóÒÈ#˜?A82³ÚÅØ4FGL J0023.7-6820?ÝÈo©ÀHJ"‹ë[-À9òóú8?âÀ<' Í|@þ¥aùÅ@›2öÍ?µp(.mQ?µ áL
Ł?ø3)ø÷Î@Gs\/¿Ðj@ºˆ'¿ç3®eÙ¿éès€¿åÀþŠÓ¿ïÿþÐñ?äñ*å†×öAGNfsrq3FGL J0021.6-6835PKS 0021-686?ïþ°ªÕ_¼?/K=P^?$õRª6?/K=Pµ?ïú`|Ì`1?bó"Ì'*"?F~Î=±?bó"Ì'*?ïÛa	«‰?u££,þ2µ?rvÏ{*:K?u££,þ2Æ?ïö_‹ø‡'?GäªT®+µ?S@èðÜÉ?GäªT®+²4FGL J0023.7+4457¿u…º1Ï#qÀ1¥3ã\[KÀ9¸AûMÀ<PZUÖ@ôrÏ«Nx@aE•6?²»®·Ë?²ƒ:\9â?þ/ˆØ6@\¼üË@?ïÅJŒì-¿ã¡Îò@û¿åÑ瞊D<¿æ‹¡>(¯¢¿é8}¿H€¿æ_AtyAGNfsrq3FGL J0023.5+4454B3 0020+446?ïýÙJš?1lX,?7_‰5«0'?1lX9?ïý§§…¨}?HîgµÜ?2ÂÃÒ¼*?HîgµÕ?ïÓIC…éò?t½^7q·6?v[^=½?t½^7q·5?ïüb¡®ª(?*tÚOŠ?<êòŠ®Ãƒ?*tÚOŠ¬4FGL J0023.9+1603?ïFÕV¬ÀG%ƟŒ!âÀ:"¬ñe2ŠÀ<s
=Ö$@É­"£:­?ÿPœÐ…¿?ǸÖöœT	?ÀxxšE'?øZÁ¶%@S$彉Ž?ïâHZ⥿ã#˜ ö/G¿àsÉøÜö¿Õƒ
¼õ¿éÕ	ÖB—¿æòçHy–AGNbll87GB 002122.5+154553?ïáÓù½üg?o‹q	j?n,B—"?o‹q	f?ïã÷ðºxÒ?}ƒÌ%"{?lE‡.@?}ƒÌ%"|?ïxˑLc'?Œ=½íFÔ?æÖs›F?Œ=½íFÔ?ïY=š`?€XcxAÑÑ?"ßxL¼ô?€XcxAÑÐ4FGL J0024.4+4647?Ôì%{¦òÊÀ/¥Þ7X[âÀ:þŠBäÀ<`;`(^Ä@½$Ö¤@Œ…=Â?Ã4øŤ"¿«Á}ä1m?æÀPQ_@	ïùÜOv¶¿àhˆ•â¿éiáyð‡¿ëEM|Š•¿ÊÐԙI聿ïÝˍ1¬J?î'¢ PØ`AGNbcuB3 0021+464?ïþááõGP?"ôŸ>ó?!á૊í'?"ôŸ>ó?ïþ‡dã¡í?E©ƒ‡?'‰±ÅáHj?E©ƒ'?ïêA{µmì?d²¼4Œ§â?e¾"J'?d²¼4Œ§Ó?ïþ¹ÇcÆ?è\›2À?$c‰Î£œº?è\›2þ4FGL J0024.7+0349¿ï75"ËÕÀM0i@5z5À:ß[†8"ÅÀ<t{i,êD@Ç-õ±q@	þCg]Ý?ÈcŸŒ¢»?¼Ù©¿Š¯?òî^íÌ!@ê0ðã­d?Ä"SçÞ¡?ï–7D9ë´¿é yó$÷¿áß-WQ­¿æ¤õ8%á¿ïóÉü7ôcAGNfsrq3FGL J0024.4+0350GB6 J0024+0349?ïþHh}y?*ÿ{G~.?+™x(g¯?*ÿ{G~c?ïýü'ÛO?H"7¹Bq?0ëñ%| ?H"7¹B‰?ïsHš'Öà?Ž-§.æ?'–ì­Å$?Ž-§.æ?ïÿ y't?ÙÔ}ç>˜?ðÍÑ¢<?ÙÔ}ç?(4FGL J0025.2-2231?ïåCû3Ð3ÀTŸ!BoçÀ;'›]:À<®ÑOŒÊ@u*ÑsP@#5ߵݝ?Âí'úÆ°(¿¢‹ìCíþ?ß¡J½éZ!@àë¡y6ù?ïÿÃF1=¿ásÁ}ä1m¿í§À8iÓÙ?°‡Ãs¢º¿ïÿØþ3w&?ïþ7ޓž®AGNfsrqPMN J0025-2228?ïý>@Fºø?G†ZGÈm?6
ýÊ(F»?G†ZGÈm?ïÝ
R?»ü?‹s{ŽXa?qzÖà":?‹s{ŽX`?Öjþd?ˆ@n(î(‡?‹Êe@f´?ˆ@n(î(‰?ïøéÛi?ImÐ.`S?OôX"žX@?ImÐ.`D4FGL J0025.7-4801?ëґF jÀQ!©æî·À:aŠ ÒHÀ<"P/Ã<*@H¹»øê?ÿm…/J?ÍiKH'áñ?Ê3E½#Œw?ÿ±¦Ö˜þ@I";ø¿çqCĐ¿Âw&gÈþ¿äZ1®
j¿ßýäqÚ
¿ë	^î¢àj¿ïÿÀ¿ù)ÍAGNbcuSUMSS J002545-480356?ïúýX.×?Fê.0éZ?DޟD¢n?Fê.0ée?ïþž³à.Õ?A6vz­&Ú?&Áý˜d?A6vz­&Û?î'Vÿáb?š©$×Fß?¦Úžpéà?š©$×Fá?ïÿC
Еë?TµdL÷?žEíB¨
?TµdMÁ4FGL J0026.6-4600¿È&	ÉÝlÀQžÏ€Ü3rÀ:Îùn‡QÀ<µG› @헗‹ÍS?þë׉¿1?Á!q)búÌ?†óxæ¤Aò?É»g_4Ã×@üe+Rê?ï÷´×ãD¿ã§E‰w§¿Þ€§ZL|°¿×ÂC[õIC¿æ›ëþì.½?®¬ù$AGNbll3FGL J0026.7-46031RXS J002636.3-460101?ïþì'êŽ:?Þy½°ˆ>?!=Wd®?Þy½°‰?ïþ5²Ãç?HzÆæu–?,¤ÓÎÁ›;?HzÆæu–?ïõ™(Î ?i§ƒÔƒ?TÍ®àcÃ{?i§ƒÔƒ?ïúýIJµÖ?3››'»˜Þ?Dí5(¨?3››'»™4FGL J0028.1+7505¿Ûø¹…l3-@(–G™ÅXÀ:Üéä4È_À<¶‡•@y56Ì?ü½3«(?ɯ_Éî?Û'‡W@
Ä_@wÏ@d
+' *¿åJ¬–Ì_À¿ê,9¿iaî¿­ª±ÄޖϿÚÛ5{Ù¿åøšá"¿ïÿGuܦAGNbcu3FGL J0028.6+7507GB6 J0028+7506?îp÷º1´?¤Él!™8'?¨ÿ€"\äÈ?¤Él!™8'?ïWz"ÍTU?¨8øxƒjÞ?•¯fUur?¨8øxƒjÞ?çŠà`Eõc?·=¼[Ÿ?Ðê??t<?·=¼[Ÿ?ìó×Ñ÷þ?dN[ˆ¨?¸aG	p@?dN[ˆª4FGL J0028.4+2001¿éè5eÎÊÀEAÑöy}À9‰þçÒÑÀ<B_•'Í@¹T
¬ç@Þ=½Ð°‡?±ÜæàÊ/º?¼l¡
ž¿@Ôøš°ðÎ@•wO>'?ïíKþSý¿áH€Âˆ%S¿ç{š—¿ãðgȖݿîÊˆNî{¿ÉxN…ÊðAGNfsrq3FGL J0028.8+1951TXS 0025+197?ïûÒªÖé?:J¢MZ?@µT¤[ H?:J¢MYä?ïý/Û¦I?Q¶ÚR]y˜?6"Í·g?Q¶ÚR]yª?ï˜qP±·?ƒÁÙC'?‰ÿ#«Ó'.?ƒÁÙC‡?ïõ3*]=R?Eµn&°Ò?U™«E…\ø?Eµn&°Ò4FGL J0028.8-0112¿ï46Ν ÀOÁàâiÀ;f؁5õ…À<œÉÄÐo@ 	{XæËü@ Ï[†I?ÏèEú
G­?wS¨ÀöLD?£É<quc@ù'#V?ïþž¹"¿èœ³sӌ¿é!P|ð§¿ÑÒ¸~âH¿â³'ÒÓø¿Üj¨ À€AGNbllPKS 0026-014?ïÿÂPe$>üƒÏ'Õ?¼>þ×Í?mÀk>üƒÏ'ÕC+?ïýÁŠ€†?Nˆƒ	‡½ý?1÷3«ûÈy?Nˆƒ	‡¾?ïñPŠ²:?föìrÖc?]^ë曈±?föìrÖt?ïý#¾5É?+p¼'Y}?6âWq³ª?+p¼'Y4FGL J0028.9+3553?‡É¹¬›ÓÀ:ÁòfºI=À:…ðÍ]…À<x4Ô#&@Ržý0ÂÁ@"*ú?Àv\¨¢v?"ib''ž?ÅAÓ_
+¸@ô1ÿ¬s¿¶Là®V4¿âcK^£#†¿è𠬳R¿ÒýcÃHê¿ëGÝ^ëGâ¿ïÿÐÀL`×AGNbcuGB6 J0028+3550?ïøÙBú?I ·7~X?Lšõ½¼L?I ·7~D?ïþº‡£B?@ßÊ%_w?$WŽËÕ7?@ßÊ%_?ïÝϧ»)^?xs^Áho?q,"kQ0?xs^Áhj?ïù?Å3?8ÂÖy‡¡=?Kë3—‹4?8ÂÖy‡¡04FGL J0029.0-7044¿ä ÖWSÔàÀG"—Oß;À9ñÇ9åÔÜÀ<|"ÿ‰;@jÆm¸@k›v¬?·»Z‰Ž^¨?¢ÿËÒ¦Ö?èfÓP0š@‰UC©M?ïÏ8''
¿æ_>ߎÆW¿âPÿÌÔY‰¿Û+ÝÿO+¿ë‹Ÿps/£¿äýÛb'ÆAGNbll3FGL J0029.1-7045PKS 0026-710?ï÷LXî?P>œ}jS?QágOÔ"	?P>œ}jV?ïýÅX›?PDþxarf?1×í;'òº?PDþxari?ïy$b8ˆï?™©ß ?Ûs¸îâ7?™©ß ?ïüeì{šŽ?/û«ƒ5(?<М#+É?/û«ƒ5%4FGL J0029.4+2051¿ïnŽ#<[xÀDÛG"#À;e‰˜š–À<¹"²²o@"töL"?öó•Þùõû?Ö"ˆô'?Óq"€¥×À@' ùà+N?ÿjDŒ¡äl¿ïß|7‰¿í8Ô'4!p?ìpéý_;Ð?ӎ˜ßŠi¦¿àXºvˆóY¿n(™) ÏAGNbcuNVSS J002928+205332?ïü<"?8u´?ì??ÏǎfZ?8u´?ë÷?ïü˜™wÈó?\æD4ãð?;;4A¸gÊ?\æD4ãø?ïÈǜtK?{Wäîžÿ?{œ1üÅÚP?{WäîŸ?ï䂵ï!?aöžÀÛÕ?k}Joß7?aöžÀÛ×4FGL J0030.2-1647¿ãN¢»†t%ÀS¤5"_õÀ:YÚ´¢À<\ãW±˜@ ŠÞOV)'?úB`²È>É?ÁÚ­àùT•?Á+"V´l¯@—ãÓs@g[¢¾Š?ïÛÛÞb¡`¿½ˆGù黿À´±øàüÛ¿Òµ(kY¿Þ×e­ê¿ÖN²?­¿ìAGNbll3FGL J0030.2-16462MASS J00302045-1647130?ïþІØM?*Ôq§mZd?.r÷'{,†?*Ôq§mY÷?ïýŠÚ$óù?PƒÏ¡?P?3©.Ø`.T?PƒÏ¡?P?ïîFk/<Y?c"Z÷arp?a¹"Ðç¢?c"Z÷ar~?ïûiÑ­xí?3?)×ØdÒ?BX¹JHÌ?3?)×ØdÓ4FGL J0030.3-4224¿ïû}(w"]ÀR‡öý!ÿ.À8â'­ÄÊÀ<1˜F³B¸@¾èÈUï¡@å|Æúü?£Hl!ޙu?ªCŽJ0%@?ÞèXD@u9ÉOiË¿×&F{9‡5¿äúNEq¿ç3SÿÜn«¿æœ}ώž¿î":귙_?ÆNÖgUN¼AGNfsrq3FGL J0030.3-4223PKS 0027-426?ïþ^Û`o?$Ŭ—ön?*N©øû–?$Ŭ—ön2?ïüç¢Áq?R³Ôï+?8ÂïIô{o?R³Ôï?ï±O¶KÌ?'ZZ"ÿ_?ƒ¬9'm
z?'ZZ"ÿ_?ïø0h\?x?E¾\¥¥E?O>^ ?E¾\¥¥[4FGL J0030.6-0212¿æ"õ»ò"KÀP%‹'¢À8Éõª;¨MÀ;ã{ÕctD@—ä´,@e…—"?§$ñž_Éa?Àpü}êg@°y=Ùc@XÕ
¥?²р)ŸÐ¿àZÖk­Î¿æ¯Ãzm"¿äqêÉ7¿ì"C çU¿ïÿ%¯¼ñAGNbcu3FGL J0030.7-0209PKS B0027-024?ïõÌE€ê?R*!O"–??Tgátþ-;?R*!O"–@?ïúu.Ûè?^=ØÁ·0?F+G̐gN?^=ØÁ·0?ï|Š©m?Œ$úÁn*?nªÝ2h?Œ$úÁn-?ïÿ%
€£×?ö:¾úÃq?^Oë…H?ö:¾úÃÞ4FGL J0031.3+0726?Ýt	&ýÀKŠýq?À:è7Åi+=À<•(+˜4?@ €³¾"æ?ý\\ø(›*?Ç/–Æ€'q?¶/O"ýÛã?ðœcÈý4t@…¼¿äqN õC¿ìàß8³¦?ãE—Ne¾¡¿èüᛐë?™<ä"Eí¿ãÕàòž™AGNbll3FGL J0031.3+0724NVSS J003119+072456?ïÿ	†PÞ¦?¾‹@ëø?Ï5ä+>'?¾‹@ëø?ïþpÕ?Åî?H&W~ñ?(ò¬¡/?H&W~ñþ?ï梽UX?qE^W"®ò?i]B盛?qE^W"®ì?ïüô*Èm?1>â{?8^¯¡¼'X?1>â{ñ4FGL J0032.3-5522?ç!¢œ‰ vÀNÆE܃#6À:MŽz¦^À<|R¢dCv@(W·L@ó•$Ý?¹JÔ»?Ś"U•]Ë@	Ëþp³Ç@¶|‰"g¿Ç
G_ɔ¿ÔÍ×ú'xë¿ä¯JÛÆdÔ¿æ+|_÷âO¿âVlSq¿ïÿòÿf}
AGNbcu3FGL J0032.3-5522SUMSS J003210-552228?ïüµ¨§ªl?@gk…du.?:RºÂ¬¤?@gk…du3?ïþBS·¹?L4²/Ž?/ëÚĄjY?L4²/Ž ?îÿ䪉Êù?"»7iB? µWcP`?"»7iB?ïÿè%TÂ=>á#'íµ>çÚ«=¼ƒ>á#'í"4FGL J0032.4-2849¿í6S›˜wéÀU^c^J8À:ã¹L½GõÀ<¿×ç³ @»ï¶ÝÍ@mnÛí÷?Äy™ßd©ù?·JÌå¤?îè³³ S]@-½@gÏ¿åÜȝ¾|¿Ñø%?–¿åÔdcP¿æ#JóCY¿é¥va†,Õ¿µËÍô?,'AGNbll3FGL J0032.3-2852PMN J0032-2849?ïñÚQ`?XPB˜o?\KÛ]?ú?XPB˜n?ïú\Ah+K?]íü—â›?FŽú_RÓó?]íü—âœ?ïˆÇlÉ?‡ÈœÿO?Î$ûͽ¶?‡ÈœÿO?ï÷XÓ¯K?D¢‰"ã	z?QáNX¡jˆ?D¢‰"ã	|4FGL J0033.3-2040?½XDs*áœÀT•zxl"hÀ;ʦ—®ÞÀ<æMú^Ö@!?Ô¶P3Ÿ?ûØdàTi?υ˜…ÈVp?µ·@Hšx'?åD¸aý–?ø‹
ë@€N?Ç#v|´¬¿ïþµbLü2?ï˟`Xy¿ÄðáxÚ¿ë_÷auæ·¿x'Úì'ä~AGNbllRBS 0075?ïý8÷16	?2OÕg
?68FvO±è?2OÕg9?ïîüðWfÍ?yåJðfû?a¨™2Â?yåJðfü?ïº ŸãU«?³=´\ °?wØ*•Š?³=´\ ¬?ïÛy) zL?jÁW(DQ|?rCkoÂÙS?jÁW(DQ{4FGL J0033.5-1921?ïð[D;o°ÀTMäÍt'yÀ8<Sz
ˆÀ;Pv'¤‰¸@p0ÙÒá?ùꍺß?¢•¾î'Å??²‹À"¦£@|¿ôw5Â@:ÁmH,ê?ãC0×?³´¬š}DN¿ÙՐàãZ-¿Ô!&€È<o¿ÝŒ=ZÔaí¿ÝV"Š‹ßAGNbll3FGL J0033.6-1921KUV 00311-1938?ïû	öA¤m?K¯çREc?CØ&ùnJ?K¯çREd?ïõbJØù!?p'@=z4?U;jN
¾Ý?p'@=z5?ï«rr¡Ì?Š öäïŸ^?…#cWŒû¤?Š öäïŸ^?ï×fÇ=y?g`½«£&?tLúaCZ?g`½«£-4FGL J0033.9+3858?ïè³Â5ØÀ7ÆÛ3—ÝÀ:h9Y½áwÀ<v[€YW@>|›Üë@Q«›úœê?Àj˜^D?©þñÀª³%?æíb6V@
¿Î÷õD?ïü¼ž×F"¿ãÆC{Ó¿å+$ p¸Ð¿çÕ)ÈPfJ¿åŽmìl¥¿èޝ´K!AGNbcuMG3 J003408+3901?ïþò#qš?1,Ùé»ò´? ÝϨæOo?1,Ùé»ò~?ïþy–ßg?CŠÆ¾¤G¹?(f'	Ž :?CŠÆ¾¤GÁ?ïî B^b?]×ʅÏõ?a_½¡øŸ(?]×ʅÏõ?ïùÄ]™P?8k¿ù•?KàÁF?8k¿ù½4FGL J0034.0-4116¿ÑOɺJ8ÀRÚu%F
¦À:}à{Ö:À<|Ïç/O@èOiõ'@"s9³õ?»ö•Žòø?"p?Ùð??Õò,'¿ãZ@‡æ¦'¦`?åÉTb,ðÏ¿åyêPì¿é'Ò§®/¿çD-÷Š¹¿ßg49eý¿ÜÙü€n¥OAGNbcuPKS 0031-415?ïý·—ëÇ?,jX¸r‹D?2CGp¡×‰?,jX¸r‹c?ïþÁë±ù€?@ó¨6çÕ?#áDàh
Ì?@ó¨6çÔ÷?ïæl@ô?k†G;,oÆ?i~"â¿|?k†G;,o±?ïÿƒr^à?ù©Š…wM?#h~Í?ù©Š…w4FGL J0035.0-5728?ê˜(Òvˆ¹ÀMÂDú<À:Ö-Ç©­À<—üñý@™ƒlÜw:@={ 1ί?Æ¢*cÖ¿?²PßkŠè|?é5Ü@W@"½a4?ïèËùo˜¿åªqѺ¨¿èMŒæ,ð#¿æ×ÔÓ+‹Ÿ¿ïþÓ°Üá?èÁ'e±ÍAGNbcuPMN J0035-5726?ïþeÅúë?/¹"§u?ß?)®C QV ?/¹"§u@	?ïØTHƸŠ?‡›D×	?sÕۜ£»G?‡›D×	?ïÍ~؆?x3VÓ`Å?y@"õ¼ñê?x3VÓ`Ä?ïäñRªs?^Ö©ðÂòg?kà­UÏ?^Ö©ðÂòb4FGL J0035.2+1514¿ãŒ7Ð.ÌÀÀG¹‰a=1ºÀ90õ üÐÀ;¾mÏç3€@Jz'ýö»?û{fX#­"?®Œæ>.û?´Àû³?2@	QÁ
{é…@
ë±îO(‡?ÚqžÞ|øy¿Ø‹MÜ+åa¿Ù8PϞ¹¿Ø(.½'¬î¿ßqÂeؿṈý•¨AGNbll3FGL J0035.2+1513RX J0035.2+1515?ïü·ÒXr?3+¥Å¼œ±?:Aom<kÉ?3+¥Å¼œ–?ïûI"2®Ú?Wç£kŸý¾?BÛw5DB?Wç£kŸý´?ïÚª¿—"?vDHò)`µ?rª 4ný¹?vDHò)`°?ïäWÔg9?RŹ9‡o?k¨+˜Æè`?RŹ9‡g4FGL J0035.8-0837¿â;"ãÙßÌÀQÈéᰉ À;[ø–2æÀ<´"Š‹ß@+2w÷]o?ÿ˜òtý?Óâ?»+åŒ?Їç^j?úEû7Cc@Ó³#Ñ¿ïý?üoQÇ?î|r!/¥Š¿Ý"m?ž{¿Ö3ªýD8ê¿å÷C~Ý¿ïüRáÏ=jAGNbllPMN J0035-0836?ïýBëdü[?9!G"®fƒ?5è¤Ø0?9!G"®f¯?ïüì÷bQR?Wi0˜C#q?8˜Díuvc?Wi0˜C#w?ïºCìãß¼?n*¦r!?oÇ?n*¦r?ïíÙ|ùÀ?Vé2í1¢?b&ƒÿ?þ?Vé2í1¨4FGL J0035.8+6131¿ÀÖÁ9»ý¿ô­6À9«½¿é{À;ZÿÁße@gˆGa¾a@
{ 1ί?ÇxÐvO'?¼Š"AeÐê?ô¶Ë8x'@
(ùÿ
È?ïÿǀ²—í¿àJú¿ú+€¿è—Z$8Ä¿äöö6R¢d¿ïúú!™­¼¿ë²u"–ØÊAGNbcuLQAC 008+061	?ïûˆÂ:f[?KçFV!ˆÀ?AÜ÷f–é?KçFV!ˆÐ?ïç$ãÕÑ?'ÂÕå²9?hÛî*.˜?'ÂÕå²9?îÌNÕUk˜?—WWA&Öy?£;ª©F"?—WWA&Öv?ïk'È
"?{šQf?'Æþ¼Oh?{šQf4FGL J0035.9+5950¿Ÿw):qñÀÖCEÏíéÀ7ñûš°À;B¬ï¡
@ $|ÍÛëy?ú•†_*2? bGÎ\š?ª¸Å-ò@
ø¤™§ÜR@'"ŽJ[?ï° F\¿Á.ÃâÃY1¿Ý­êžïÄÉ¿ÑÓ
X®ÿ¿ÛB?•—,¿Öîï!
'©AGNbll3FGL J0035.9+59491ES 0033+595?ïþ½ep?!Î5­3?$)¨÷3œ?!Î5­2Ö?ïú^Û
¢?iù$)x6§?F""Õw§B?iù$)x6 ?ïÄ¿è5]Ó?³<ȱ9?} åQ¤?³<ȱ9?ïüŽFRcÚ?-n6ëx~?;Ílá7Ó?-n6ëx~,4FGL J0036.9+1832?ÔzBWEæÛÀFÝ/Ÿ¾À:Yºû1À<n}îBh@g*&š£@'L©%þ—?ÀCW÷ã§?¼Ìõ''5?ûz&6Ën@ªk­Î¿æÚ³ì+¿àú®/«¿æ,@Ъ¨¿çÞ¯°î¿×)9_G8N¿ïÿÁìžú,AGNbcuCRATES J003659.39+183203.7?ïÿn'""D?¶¤êzû@?;mwZp?¶¤êzûÑ?ïýäOr€u?M·sX^¬ô?0݄kü^?M·sX^¬ï?ïàc•Ó0§?n'9m»\?oœj,ÏXŸ?n'9m»^?ïÿÒDªöG>v‰>öݪ"܈Ë>v4FGL J0037.6+3653?ì`Ÿ"\ôÀ9ä—{žÀ:ÌÿؒӭÀ<t1rhÓ(@ÆXIî@$UšfH3?ÉÌS•©J?»zàÆÔ».?ðÇ#Zx›@Dt€ª_¿í¾ûˆ¡ú'¿ºÕ¢"C¿åÑÁD®[¿ØkYë-àä¿ìmˆcç0%¿ïÿÃßé47AGNfsrq4C +36.01?ïôi{·ù?Xu½ÿ$Å?W-	ސ	l?Xu½ÿ$À?ïúŽIg#?[꺘±ÿÄ?EÆÚcs¸ù?[꺘±ÿÀ?ï‰^`p¤Á?ˆò•û_±?¨gãÖÏö?ˆò•û_´?ïÕ¿B»…?eŠ™: «O?u ^¢|=—?eŠ™: «O4FGL J0037.8+1239¿¢®X½QûïÀI
¥¤i×4À9€C`§à"À<+»Ù_'G@¶I'uç@ÁªYÛ=©?­²ÿµò¿rÔåþªä?ÃÓ·79R1@z~ædùT?ïÆZAêÜ¿â咖pn¿ä›:]ôÒпà+Ôßë¸u¿ãÏß Œg'¿ã]åÄ—gAGNbll3FGL J0037.9+1239NVSS J003750+123818?ïý¥Zqä?/''Ýï?2Õ,pß[?/''Ýï0?ïþ‰`(å"?A‰°¦üÉ-?'iýq­à?A‰°¦üÉ=?ïõ§å2Õ?Q`¨sëÿ?T°5šäW¿?Q`¨sëð?ïÿC}¨˜‹?
%þ"]øt?Jìî¾ý?
%þ"]ùÉ4FGL J0037.9+2612?ï6›h
†ÀBI/Ÿ¾wÀ:×Dœè³À<ˆ')ó@+QّG@ì楻æË?Ì.sEqú?Ã'À²7J?óŒÙ|Þwð?û҃Ee¿Û@`óJ:¿à'È>Ȓ«¿ä¡wÿ•÷Ï¿è"J½¾g¿é.†%HŽå¿ðAGNbllWISE J003719.15+261312.6?ïô±
™?UTKnC…?WƝëðÐH?UTKnCy?ï}xQ—B¤?¦¨4'°àT?PõÍ«ƒ?¦¨4'°àT?îÔ
ã!ào?"û±ÉY?¢¿QÍáù?"û±É\?î՚¤Q²?Žàt©ÓþÏ?¢¦UºçË?Žàt©ÓþÑ4FGL J0038.1+0012¿ëýò,McÀO<±î$5iÀ:úûö†À<_zù›añ@»…øÒå@
¥|üªá?¶	Ê?eò?–õxί?âp¢qON@ï72œ4¿ç•¿x¿ØCûlóHb¿åCW}ÀJ2¿Óîᵒ¿âvOb=⺿â˜H+ü'AGNbll3FGL J0038.0+0012NVSS J003808+001336?ïõ
ö?QĦg'?Uê Ö²N?QĦgz?ïûÜå`y&?X{̬:?@Œj~fB?X{̬J?ïÙÝAü2c?v_|Sª 5?s_æÎU?v_|Sª 2?ïæ׶êï?[Þ|Ÿ(ö?i(Ibå?[Þ|Ÿ(ü4FGL J0038.2-2459?ÞúÔaÁÝYÀU–Y_í¦aÀ8ùþz¾ãÀ;ùž$BÕh@8ÃäpØZ@Q¥Ãsˆ?¦e¯¡º?¶ÎQ ï¿@aƎÅ*A@žÌíY	\¿³ÍlÚɺŸ¿Û-+|…Œœ¿äï4 #b¿âˆõý¥¿ê@N¤©¿åó4«wªAGNfsrq3FGL J0038.0-2501PKS 0035-252?ïúXĤ€?@A:¿+Ō?FœímýÂ4?@A:¿+Å?ïü$Ä:æ¾?XG"–}ZC?>ÙÞ(ÊÌ?XG"–}ZC?ïUo<5Éþ?Z·Æs?•RyFÀ8?Z·Æq?ïÿüÙ«·>·~ƒÓÅ>¹2§HMw>·~ƒÓ5©4FGL J0038.7-0204¿ç[wBRÏÀP0¬![š[À: ñ68¡1À<F"—u@Ëßèˆj@÷ÇÀ?Åd¦¹
þ?̟6çrÀg@öÇd­ÿ'@óœÚ
οËB#;"Ü¿æBM'iÒ,¿ëÍQŒºŽ¿ï݄?•AE¿ïž©£Ò؀?Áþ0\"*šAGNrdg3C 17?ïï떛]?gÃöktU?`id¢ý—?gÃöktZ?ïµk$Hp'?'ì']•Å?'¥6íã۝?'ì']•Å?î3vœn÷B?	ì2ø"?¬È–9‹ç?	ì2ø?ïvÇ-L ?Yà%­¾?''V»å?Yà%­»4FGL J0039.0-0946?î9{"ÆÙ¸ÀR,ºËCÀ:#ª–A…À<f=°d·:@é3þà\@u{­ˆ?½í'þŘP?¹PXÝç§?öüºÑ!Æ@û!'ÌËË?ïÿmh¹&þ¿ãšQ_™¿¿é5Ù L£¿ètSß{%:¿ïÿñ_{'?í(#ÕÈAGNfsrq3FGL J0039.1-0939TXS 0036-099?ïÿKÓâé? ëe ½|,?…ƒ½Â°? ëe ½{ß?ïÝë¾Ë?…–¾tµR?q@|Š šÀ?…–¾tµR?ïÌÏ­EÇ_?z_Eº,?y˜)]P{?z_Eº,?ïÚ\@ïœÉ?fü°ë?rÑ߈1›?fü°ë"4FGL J0039.1-2219¿ã?uú±¨ÀUg8}¿À:…®Ús~}À<o­é¿@ ÚÒZ*mè?ü(—ξ??½
díj| ?sUÙë9I?¶©={‹'™?ÿ–ãìÎõÇ?ïàYÜë(¿Ö8è^£¤_¿Ôb·ðœµ®¿Õ1fªY~¿ãZ7ÿuÁx¿ÅíQ½ƒAGNbcu3FGL J0039.0-2218PMN J0039-2220?ïû­gµŽi?9)Æ÷òÃ
?AJa)ÆW×?9)Æ÷òÃ?ïúk'ÎU¯?[]WÁ~?FQ¸Æ©Aò?[]WÁw?ïíØ+2ç$?g¡¡ú'?b'ÔÍÜm?g¡¡úŸ?ïç}kü?Z*l?ýŒ?h'ãþ"€?Z*l?ýŒ4FGL J0039.1+4330?×*²yïp>À3M½ÙßÛÀ:¾ü‡7À<žÿ%­B@yl®)@
  ôØ?Äa1s?'½?Ú6bÂö?ýàõþõ>@	·"W`9&¿ì²ÊÃQ-?ïùZ"¡U¿á­,ˆõ¨¿Ýe¿cØ¿à/³KòG¿ïÿ8"†ZAGNbcu3FGL J0039.1+4330NVSS J003907+433015?ïüÚ*Êþ{?5™,«=¢?9.©¨[?5™,«=¢?ïüY®ð±?Vˆ³–N?=2ˆuf?Vˆ³–N?ïښ½ò•?rÌ4R.v?r²¡vµÖ?rÌ4R.v?ïç[ÅOƒ°?Y6'r0¥»?h¤:°|NÁ?Y6'r0¥Ï4FGL J0040.3+4050?Ñ*e(
žHÀ5ü¼ßï¿@À:¸Ø£š¤À<zøØÄQÔ@!A߇O?ÿ¿ "_õ?·[±×~·¿³0M¿jRs?û-
ê¤N)@b14?èöIØÃ{¿â6M™æÆs¿èê"‡¿R¿Ö^¿à12I(h¿Å"§ŸÁ¦ÔAGNbll3FGL J0040.3+4049B3 0037+405?ïþ u½›ž?+uZ>#Uˆ?-ø¤&Fä?+uZ>#U•?ïýÌZÿ¯?K
&aâ=?1(†ÿJ?K
&aâN?ïð¼Ë‡Á·?nSÑüø?^†hð|'Ñ?nSÑüø?ïäu¢`Úq?Xæ«|ÕÓ?kŠ]Ÿ%Ž«?Xæ«|ÕÌ4FGL J0040.4-2340?ĄMóhõÙÀUo@öjUÀ:˝_÷·À<š/²u2²@ÍÛLlj6@v¿yýòà?Ædô5òUH?ª"Ù…xO?ãl Åre@3¶-y
¿ºÔ뿬'ç¿èk"\Ì4¿ã³A
ŒK¿é}ÉÄڐ¿ÉÕdK3'¿ïÿס<%JAGNbll3FGL J0040.5-2339PMN J0040-2340?ïþTÚoÛ8?%À`ñŸ§?*²YL}Ø?%À`ñŸÿ?ïþ#h¾?@ÔcVð?'
É~dý?@ÔcW?ïèìô+?j@xhLa?gäÔr¤?j@xhL`û?ïþ¬ í?$µ>œ¨?.=ñ(¥?$µ>œ¨œ4FGL J0040.9+3203?â+©·•^ˆÀ>Ä(äû—»À;ðR
À<]J]ò$@Qmª'†W?ÿ–»cýM?ئËEäß?àEÜMsPZ@ÙÂbæ@€ðâUË?ïøIóiȿքÖ~|\È¿á¬btx¿äÏìÂ5š¿ïØl:¿å5{!ŽAGNbcuTXS 0038+319?ïìÅé|®ý?g{ŒÐ"£?c:ƒQ¦?g{ŒÐ"¡?ï黏g	?|sLÿ—?fDp˜ñö˜?|sLÿ™?íöÒÐz?H³Ô.ýˆ?°IiÜ/ö?H³Ô.ý…?ï%K;5´€?…ñ©ýùj?›V˜™Ioä?…ñ©ýùj4FGL J0041.3+6052¿åðÓ	›Ò¿ÿƒòÖKÒÀ9šN³Â9ÌÀ;Jˆ0»‰®@5T#sø@ä¬å¦¸f?ŲºÒÏEM?áúˆÇº>U@‡žYòº?öY0³Q%·¿Þ–ý]
w7¿Ë$úì.'¿èÕÃ"æ¿îÎR]ðÌ¿ämÊ=¦S¼¿ïè/>\;AGNbcuNVSS J004058+605407?ÎäýKû?ÑRN:'5?èyúFÀ­?ÑRN:'6?À
({3j\?Ê;€TD.?ëüµá3%i?Ê;€TD.?Ó¤ÞÖ »?¿R¤³L?æ-"ïø"?¿R¤³K?p+uÍËc?b•ÙOd3?ïß©di;?b•ÙOd34FGL J0041.4+3800?Æý±7°cÀ8ÑüÁr&À;ŽK^À<©G_ɔ@ ÉfI
5
?ÿÉT!ÀD(?ÀU€ÙÚ&¿­§¤|ÕX?ï0\S½í6@½ý|(?쀏qøjà¿äŠ:N¿â֘B"пä÷bØ<l˜¿ÕœøÞbK¿Ä1ƒìÅLAGNfsrqB3 0038+377?ïü`çè0Í?8]ŸCˆ?<øÀ¾yÏ?8]ŸCŸ?ïýJ…æEq?b[Q¿W>{?5«ÐÍÔw!?b[Q¿W>y?ïðúj=Ló?g*E»™_?^+…f…?g*E»™]?ïò|Á +?H͔e†J—?[Ú}¿¨Ÿ?H͔e†J§4FGL J0041.7-1607¿âÃÄúÀS±úëÄ	À;±¨´¿ÍÀ<ÜøÆOÛ
@!ËXàÁÌ>?ú;´4çh?ÕغEºÊ?ÇÉFZ'W‰?öIŒ\`S@DÃàj
?Ûö'¡þm?ïúeµ²¿äå\{+‰¿Çܺ–}5¿Ë­šW"¡:¿ÖÖò FAGNbcuGALEXASC J004141.24-160746.6?ïüc,ʏh?9]D)¹­?<晫"µ6?9]D)¹§?ïý©%¹?K¸¬÷Ø<?2·¦Ò8v?K¸¬÷Ø*?ïÊ4‰®Ä?z¦w±?zå»(úº?z¦w¹?ïø¦Õè?Daò"¼ç?MgÀ«¬]ë?Daò"¼ï4FGL J0041.9-4702?ïNÑ«‡ÚÀQ­À˜$À;ã‰>ÃÀ="ÏÝù@ Ÿ³-¿Uì?úõp	}WD?Öí!zN%?ËD&J—}á?òò<ÈÞ*Ã@hÍ¿ïÿü¥¬¨¿ä¥AØèd?ïÿê›ê¬²¿Ýó"Çz¿áY®Çÿ¿Þž¼n/ÞAGNbcuRBS 0097?ïý Õ]…ë?6ô³Îˆ‹ú?6ùUН??6ô³ÎˆŒ	?ïüÏW©å—?S}CaÛ×>?9…B°ÓCê?S}CaÛ×1?↑Ílœl?€‡™½#¥?€L¤Øåc?€‡™½#£?ï÷Ȕ®VÆ?CšU9h$Â?PnÖ£Rq€?CšU9h$Ú4FGL J0042.0+3640?¿gÈg½5À:)/ ×{|À;ò×ùP¹À<Fyaî@È)NWüÁ@ç';®+ø?ÃD&àêf¿ªñ/؊Æ?ËA˜¦ªy;?ÿ¡W¾'Ý?écànë?î¨ü
,8m¿ëŸ|!Ž›¿ÑÎû%OÅ»¿ßÍã£(
»¿á¶Í§%sAGNbll3FGL J0041.9+3639RX J0042.0+3641?ïï|Ñó'Û?[öpáY­?`ƒ.Ø#Î?[öpáY´?ïú%†¨?i‡íÐõ:?Gã·iåbA?i‡íÐõ:?ïàÿA#ñ?i=ûâ•Ë?oï¾ÜŒ?i=ûâ•Â?ïÃE·%÷?jKlI/?~]p¤m»?jKlI+4FGL J0042.2+2319?æI…ÄâPÀC¿rÅz%À:#ŒÍ}À<b Õb"@\*2	h@Ö×¥mã2?¾‰_d¿rF?¾Òo_DšJ?ýzŽ ¿"(@ø­ˆÛ0¿Ÿ»Þ#G"ú¿æ²g'Ñ`¿ã$e¥vF®¿äšŽ:!¿è@*'_–>¿ïߏ@zAGNfsrq3FGL J0042.0+2318PKS 0039+230?ï}<.H¤A?˜ jñd°?Xz6ëwÑ?˜ jñd°?ï÷ƒ¹íÜ?e¶ù#v†ö?PùŒ$Hó?e¶ù#v†÷?Lð\a?ˆæ¿VTe?‰ìÃèçõ?ˆæ¿VTc?ï–GÜ?s"áhÐ?Š{¾{.	*?s"áhÐ4FGL J0043.5-0442¿§´]‰ûÀPߊ\å´$À:æ~Ä+=›À<†,:ñn@ š:ë
š?þ Aׁ\?ÆÐ\cÙ`?¤âcâÓt\?á­»úíqˆ@""xB[ð¿ê?.8¿âÑBþ,kC¿ã'·iŽ9¿Ö
×YÉ¿àý­_Ÿ!ï¿ÍïªGfÆÞAGNbll3FGL J0043.5-04441RXS J004333.7-044257?ïþÂC¡–?pàb:¢?#ÛυæªÌ?pàb:®?ïü²'y}é?QÒ ƒž/?:nÄ4º÷?QÒ ƒž#?ïøå­Û"?HsevèJ?LiH'ï²é?Hsevèo?ï÷"K…¦?Dz—'Ïx?P×hô³Ú¥?Dz—'Ïu4FGL J0043.6+2223?ØEFÌáesÀD9‡çÀnÀ;¡"úÖËÀ<'g†!Ñ@†Ã>@=–é»ðÜ?Ò£9UŒ$?·iþ Õ®?é=[?Á¶ï@¾†ù¿ïØ ó•Žr?ïџD~_¿à¢wžÈ·¿ß.8øo¿áéBžá7¿ïþΈ°=AGNbcuTXS 0040+221?ïþѼçrh?"›øá,bÙ?"ä1ˆÙ‡¯?"›øá,bÃ?ïþ¸öÃ?FPw] P?/ÄpŸ"ãK?FPw] .?ïçœø"k8?l|h°Â†?hc{"Ç?l|h°Âx?ïïîFVÖÍ?Qv.²IÎ?`¹©)2Ÿ?Qv.²IÎ4FGL J0043.7-1116¿ïD"†J®ÛÀRƒ7u¸À:șI—#À<ˆÊ½ÿ@ )Ð3Á?ùz@Ù#¯?Óì'?
?Ñ"‰âíJœ@¢Pr[@}¢×/ý?ïÿŸ¸fä¿ëa¯ÐâÜ¿Ù5 uÖÇ¿Êò*Z~&¿æØåÿùŸê¿ã‰!Q^lAGNbll3FGL J0043.7-11171RXS J004349.3-111612?ïÿˆ]¹qE?
Î×4K?
董®ùl?
Î×4Ka?ïý­Qbu??K<B0?yf?2•tìVè?K<B0?yx?ïÔÅÚþ•'?xhRùZ±@?u€µ6Á?xhRùZ±6?ïìíÚKšÿ?U,»´âß?c%´e4?U,»´âä4FGL J0043.8+3425¿Ê¹IÃW>"À<j|¦CÌÀ8b–›¸XÀ;'U¤wC-@^[/¦Œ?ýÓèPïÝ?¡kÉýQ?ªs‹_fN@
¾•ßе@ýýÃå~?ïÿG©ýd¿Ø\4ß/ÐÓ¿àíØJ¯P»¿Ù·ã܈׀¿âÝÞQ"'¿à°éAw™•AGNfsrq3FGL J0043.8+3425GB6 J0043+3426?ïÿr™°é?÷zòƒÎ=?¬Éÿ¢ý8?÷zòƒÌ?ïüŽk)W?S´ˆ'¨œ?;Œ§>µI[?S´ˆ'¨?ïÝ/q±??t€2r~…«?qhwG'`u?t€2r~…¯?ïþí?=½ÆouÈ?.Ρ'ïÕT?=½Æou¤4FGL J0044.2-8424?™q=ÅA/À@\¤~Ïé¸À:P"Þ™À<:Dfa]é@Ä9Ö:Š@JCþ\'Ñ?À4	òÈ	?1SW''»?ÐU@0ÞP^¿ßB™¢ÓÔÿ¿á€Ì¥Wh¿èˆ^Þ²¨¿ëÙY_ç¿ÇbT]û2ç¿ïÿ`}™2ìAGNfsrq3FGL J0046.7-8419PKS 0044-84?ïþþëœ|ý? ¢×
NÝ? F80"? ¢×
O	?ïþáãÆÊ¢?@U°ÏËJ›?!áÓUá?@U°ÏËJ™?ïãeœ;?màžN­-Û?lšcĀé?màžN­-ç?ïÿ±o"ß>ù¾X?¼äȀU>ù¾X4FGL J0044.8+6802¿ïR{M'|S@²{²þÅmÀ9ÈÇÜ$YÀ;¡óÒvZ@ו#SÀ@N
Ää ÿ?¿TWñ?³S¡èÅ?õÙ	†'@éšòŠ «¿ÕßGŽ4
Ê¿ŽXkã=í¿éùù î?¿áx7Ÿ(¤º¿æPqgKh´¿èë»MlšAGNbcuLQAC 011+068?ÁŽ?í•Q{?ŠºÔÏ¿œë?í•Q}?ïÞÈèïtµ?‹¦+«˜°r?p›‹ˆE¥?‹¦+«˜°r?î¹&Эû?œÒòVÇdØ?¤mž'õ 9?œÒòVÇdÑ?ïoFن‰I?~X-žëCß?'$Ï.Öð?~X-žëCÜ4FGL J0045.1-3706¿ãQ>Ürè7ÀSûί%À9µ@+i:VÀ<†ãlK'µ@çoÚX|@¡–EQBé?®©é…Y?™€öà^?çœAƆ@†¥ªõ·¿ÏȆŽàÙ¿æ4B'KÇ¿çÖø4Y£à¿èå—ží–¿ì '¢ s¿£.üÓТAGNfsrq3FGL J0045.2-3704PKS 0042-373?ïÿ
OEð?zÆP •+?¶Máǹ?zÆP "Í?ïþÅüː?KØéÏ`É?/ã 3Fô/?KØéÏ`Ó?ïê†20ö?a¾dâ˜@Î?eyÍÏ	úx?a¾dâ˜@Å?ïÿÀ?úê¡>ö2´†"éc>ÿàŠ®Úð>ö2´†"ìt4FGL J0045.3+2128¿¸^FÀ[ýÀD°üó0À8Ýi¸*~YÀ;œñ-Õ%a@¤zŽ¤h?ú´‡Ç	>m?¬º¢}ÃÐ$?³ˆ¹ø^Ëè@ZÂß
A1@žA|Í,?¹Jˆ ‰3+¿Ø/õ;*ùS¿Ùåpݍº=¿Ño¤}£Cç¿â9ʑ‰)à¿ÕT•cT
HAGNbll3FGL J0045.3+2126GB6 J0045+2127?ïþùð.t?•ë¹j? `ýˆÔn?•ë¹ú?ïü¯ºÛ¬?Sâýg‹?:'/é"²i?Sâýg?ïæÑë§j?l¾ÊMå4?i.íX•Ñ?l¾ÊMå5?ïÿª
§s³>ú¤Ä•5
4?|–#R¼>ú¤Ä•5B4FGL J0045.7+1217?˅îBäÁÓÀIGD#‰À9QË(‡Þ†À<IbI¡4@¼ÇÞ{uí?ÿPUhaQ?¯<òN¼{œ?•(%Ž.?çs÷+E(@ÿz'î.Ç¿ØPQÜÁŒ}¿âI¾ó(¿Þ¯îºÞ7Ù¿à')ÜÓ¿×âš~ñ͍¿ä[³"ý*cAGNbll3FGL J0045.7+1217GB6 J0045+1217?ïþB¢òi[?!çE¡¯¾?+ÕÐÙj>®?!çE¡¯{?ïþ
a¿¸}?Jåޘ¢?/)äx3©?Jåޘ¡ú?ï÷
¹ëóõ?\±.Õݹ*?QäŒ(Ä?\±.Õݹ?ïþzOxy?1Õú°'?(^›xŠ'?1Õú°Ñ4FGL J0047.0+5657¿ïb…ÔL #À 2@Äì.À9'RYi'âÀ;áJóCY@Äé÷U @"úC'œý?³õõ d4Ä?½ü`‰ê
@	,žÄ{Å@ý¢Žø×?Ôy™ž÷ýR¿ÔúŒ"¸'¿á»´v"±Ó¿Þ­' ­ßø¿å`s^™¿è fèlAGNbll3FGL J0047.0+5658GB6 J0047+5657?ïü	&WO?:ðéìØ¿I??¶Ï
Eþ?:ðéìØ¿?ïû•/U½W?^¸xµz†?A«B©
¥\?^¸xµzŽ?%bà?ъjU¤?~¼¾mNÔ?ъjU­?ïø`¦¾7?:ßᾕ?N}gùù?:ßᾚ4FGL J0047.1-6203¿ãyIb¿tÀKˆÎp:ûÀ;3&yÀ<‰ÿæՌ@S1j0Jv@	]"à¤ñ?هö#]RA?äiTpš?ú¡#K^£$@k%mL߂?嗀Œî;¿êŒºùe²¿ïü£õ=._?íSÀì÷¿ïZ¿Ï
o¿íã°> ÍAGNbcuPKS 0045-623?ïÄn*N8?‰sWDFX?}ÈêØòãY?‰sWDFX?í×tL¿~!?ÂR¶ 6"Û?±D]šþ?ÂR¶ 6"Û?ìiãLßÁ?¤?æÇ0S?¼°å™÷(?¤?æÇ0S?í jMÜAŽ?¹ÿW»f&?¶ü­'óŒ?¹ÿW»f&4FGL J0047.9+3947¿îL~vÀ7¶o"5ÒÀ9uÓú¾wŸÀ<*¯ZËþq@¬Ë"œ?ÿ1è_ÐJ0?­óÆB"?œi³Å6Læ?ðw_²íþ@»4‰tˆh¿Ñ	£¢†þ¿áHÅ †l¿ß®¬:Ûô¿ßj
 AÿT¿Ûä:|¨¿áª	µólAGNbll3FGL J0048.0+3950B3 0045+395?ïÿõâ½?õ ôJv²?C°`?õ ôJuÏ?ïþyºÂÿ?Bya;Ÿã?(o¤Sп?Bya;Ÿï?ïõ`éé?`
´[•H?Tý?Â,-»?`
´[•P?ïþÅi¨–?óÀö¬ò?#©evŸ?óÀö¬R4FGL J0047.9+5448¿ïزÞyîÄÀ "q›MÏÀ;MHœQÿÀ<¥;Ϲç@#—/£†­Y?ùJ?Ú
¢ñ?Å …œº¿tˆÏ-5~?º´÷ Þ@íšü?ç–º$Sœ?ïþ¡ÆŽÅ*¿êZ^gŠS?âúÎÓ7J¿Ý=–ä]$¿ÆÑ>¶ôô3AGNbcu3FGL J0047.9+54471RXS J004754.5+544758?ïýÍúÏ^?0 ñÐXîª?1/)…'?0 ñÐXîÚ?ïý$eTYG?Zà¾¹·?6ÜÕ]5Âñ?Zà¾¹·?ïÖ_›ÂQ?x€g$àÁ?tÐ2pž×ê?x€g$à¾?ïñc@u}?U®?ú‹P|?]9çØ?U®?ú‹P'4FGL J0047.9+2233¿éËÅ'\ªÀD&™Øƒº4À9àGÐy)¸À;é•é
ðõ@H	 <Ëã@åäËÇ?··Rèa?Žá‡Ÿ¤©?ØÇW­eÿ8@UC#Á%O?ç(å!,u¿å˜|··ð¿è¯;Œž"¿â13~²†¿äñˆ£¨U¿ïþÛÝáÈAGNfsrq3FGL J0048.0+2236GB6 J0048+2234?ïþ1Ø$].?$õ2ue?,â}º-&ù?$õ2uý?ïþxlÙ]'?A0­ÓR§?(y2j-˜?A0­ÓR¹?ï×ôIa?sý>+zB?tðð[O¯?sý>+zB
?ïÿÁ^ô>ò¾ˆJU+×>ÿP…ÿ¹‡>ò¾ˆJU/4FGL J0048.6-2427¿ï+҄=—JÀUÐQ£"îÀ:×{‰äðÀ<¦WF7ò¶@Dú¦#ë˜?ÿ¡¸·lx?Ä~´%Œª?º5‡Ì<¯?õ®žä\6@VÇâØ'?ë1` (Õ¿ß[dc¿àgN"¢Â7¿á÷7…¨K¿á¥ø¸
"'¿à_`îWaAGNbcu1RXS J004836.9-242631?ïýÀ/½v?-­ì:ð?1þ‡'Tr?-­ì;?ïû\ OòÜ?[Õõ9O}ô?B~À4Œ?[Õõ9O}÷?ïï4{]º?fúx'ÐÁ"?`r˄¢F@?fúx'ÐÁŽ?ï麌nøž?VO.1 XŽ?fEs'bœ?VO.1 X"4FGL J0049.0+2252¿î^ÞLuËÀCÿU›=ÈÀ:Ýeõ'^êÀ<<À%z@éíÞjY@œ©ïR2Ó?Ê ½šTÕ?¥‹"òe¸—?ÞVq[Œî?ÿ[ˆdpm¿î`ýÀµ'?ÕéxÔýó¶¿é#"¿lçà¿âü	Ñ:׿Øã_5o£¿æ}ÆUˏAGNbllCRATES J004901.37+225315.4?ïï7—ÊÊî?cÖ¡)Ç; ?`Èh55>?cÖ¡)Ç;ª?ïø¼îc??j‹´FáÐ?OµFsø?j‹´FáÌ?ï¾òp†?ÆQ ä?€{z#ÞA?ÆQ ä€?ïÑ
?kõ"ÎÅ$?wzô¦¶ð?kõ"ÎÅ$4FGL J0049.1+4223¿ïö¼šyÀ4zÅ;ËÀ;*|næg©À<³ÿþR€Ö@ ×âæê…D?üQ¸> NÀ?Ó Iaûc?¿ ãdéº?ï-Ú-Þ_œ@|Eœw?ï¯2Ú˓¿äut¡<¦$¿è$cÂG7Í?"UM[ÊÎg¿á¿m~2µà¿á6ߐðAGNbll3FGL J0049.0+4224GALEXASC J004859.14+422351.4?ïÿ´äHŠÎ?…Ãœ½ì?ÆíÝLÀ?…Ãœ½¸?ïýðò}ÚÉ?Q;˜ô²?0xl)°Z?Q;˜ô²£?ïñjêAc·?jÞ¾kënG?]*+}8"·?jÞ¾kën7?ïöèD:x?BgڀÑ?R/w‹Ãf?BgڀÄ4FGL J0049.4-5402¿Ù÷47ÀPÀO‹e<š»À:v©ò­1À<®Ð"¢§@Nu*¤n_@j<÷T?Á¨òÒðÓ<?Â.À‡ÅÙ?ý­X"?…@n>§Z¢c¿å3êH֎¿Ü–AöD•[¿áM¦ a4¿áVÊýiͤ¿ã±—¢H"Ä¿ïÿæ4|ßOAGNbcu3FGL J0049.4-5401PMN J0049-5402?ïâ4Y/`?l±§å¼‰-?mËæ¦Ð '?l±§å¼‰2?ïølÂO`	?`¿óG'2°?NLöÂÙ ?`¿óG'2°?丹D"´ ?">·¦˜u?†˜n÷R×ô?">·¦˜u!?ïÇd8ϏR?j<l"ˆ??|Mã˜8W«?j<l"ˆ94FGL J0049.5-4150¿ìؓ¯'^ÁÀRÑÀÁü2À;pÝF—"À<ÛÓÜí@ [k¤hՁ?þìZ{v™?ΒÉ[S7à?¬RÚ?âeIÀé>È?öÿ¶ßO±C¿ïýà5_]^?ﶴÝlØ¿ãN$ É8Ä¿áÅGMƒA¿Âh±Å4}
¿æ%µÁÃY\AGNbcu3FGL J0049.4-4149SUMSS J004938-415140?ïþ!ïÀj?1¯GeV?-áþyPX?1¯Ge'?ïð{¢Ös?yK"@tý?_ºSáõ?yK"@tü?ïÕ-PsÛ?v+{†ƒˆ?uiWôÆm?v+{†ƒ€?ï×õ7ljÉ?iIBE;¶Ö?tdIʛÍ?iIBE;¶Ï4FGL J0049.6-4500¿æ'Æn«´¬ÀRo~=ÁÀ:ØúÕS"À<©"3(Ky@NÇÉ-@©WÚ²h?ÇlJ«õ½?®»¬¾åXŠ?㟮†¨Y@Óz›§Ó¿±V
þ'¿æ̬€üꢿç{é»â¿çk|·¸¿ïÿÿ" 5•?èiÇy¦µAGNfsrq3FGL J0050.0-4458PMN J0049-4457?ïö×|7ÃÀ?YFÄüs
?RQx«?YFÄüs?ïÙ,)²?‡©ŸÆµ?siüëp&}?‡©ŸÆµ?ï´¬/ŽŸÅ?|‡ŒÊk®´?'ÔôXÛ?|‡ŒÊk®¶?ïâðù^¤?`æ°"ÍÍÊ?m¡ø[‹?`æ°"ÍÍÐ4FGL J0049.7+0237¿ìöÙÐR¡2ÀNï
å6PÀ8íeéŠsÀ<	"¾pé@° í@P'½´+?¦\‹œ*îk?­ODœù0¿@CjÆGwŽ@þÓºÒ¤R?á' ù	kº¿á'[åY¿ã›.Y¯ž¿¿ák7†
¢¿è'Ì®š¿åÀ×@n/3AGNbll3FGL J0049.7+0237PKS 0047+023?ïûød}Ê?7ñ%šÐ>?@oæÓ$?7ñ%šÐ4?ïýS²±S?LvÅm@fg?5bjugg7?LvÅm@fn?ï³2ØÜ¡?ÿÿ4i?ƒ>sIÈ×â?ÿÿ4a?ïüûÃá¤-?,R'cè´F?8!àòޒ"?,R'c贑4FGL J0050.0-5736¿À3eݶÀMÁe^(ªCÀ9¾®"½š*À<gKrÅz@k"K÷¥@äwC-|:?°ZöƛZd?f7þ…<Ñ?ÎVüfŒ@¿ü'Çðð¿ÎÑèÀsM*¿å!aña­¿éÅ%nO¿åÀ–'õ¿æQtœŠâ¿ïÿ¢AÞÇ¡AGNfsrq3FGL J0049.8-5737PKS 0047-579?ïÿW_mã?øH
šä?ÕCˆÍ?øH
›`?ïþ1¢:¶?I(1ò¯"x?,åßüTÁ?I(1ò¯"€?ïäð‰UT­?l(Ug?kvª«Sk?l(Ug
?ïÿM!<$c?
7IvðZ?[Ø{sˆ?
7IvîÕ4FGL J0050.4-0452¿ïÞùŸéÀPð¼£À9 ܝ$h•À<cæYeÍ@"Eò¨@¯ÁÄ[D?«¿ gå©?±·ðq@­¶åû7@R҄ǥq¿Ïá
?x¿âýW^‹¦'¿æOµë÷ö¿áï åRÖ¿ì—tË"¾¿ä¡Z=c7ÞAGNfsrq3FGL J0050.4-0449PKS 0047-051?ïýßź€?0¢Îü˜Öâ?7)Ò,õ?0¢Îü˜ÖÄ?ïþ'£òš?A+w¯i®?'ÕÀÖ^µF?A+w¯i•?ᅭ橏Ô?/J'+Ð?€FUœ?/J'+Ï?ïÿWÙáë?´NïÛ¾!?߃®í?´NïÛ¾³4FGL J0050.7-0929¿ïlÝú緑ÀRSÞ¤e¥À8Q'M›À;\ΌÀmC@Q(ÜC?þ¼~ ïÏ0?œ‰8DâT–?¯Ið !Ú,@§¾öJu@?¤T¿?"Ç9¬L­¿×£I›ªjø¿àø%
{"¿ßÛ¿PãG¿âiTWp)^¿åP}'%VÒAGNBLL3FGL J0050.6-0929PKS 0048-09?ïþ¨ž¼sN?' ŠIåt?%v8Ëé?' ŠIåí?ïøÜ	Rê!?cïkQD§+?LÚ´Wz?cïkQD§%?ïÊ:rL}Á?€ÿÔ c—Q?zâÆÙÁÚ?€ÿÔ c—S?ïøþxŸ8~?:=ýÅ÷A\?Lƒ	 ?:=ýÅ÷AT4FGL J0051.1-0648¿ïm†½""¥ÀQk˜ñÓíRÀ9r}7%À<©&¤¯@€|ªEä@ÜIwBV½?±üàeÛÑø?ÃïÙÂ(¯@ÔçhY…­@Sš±ÇŽ?ïøÇǪN¿á½KÙÅÚ¿ä>Ðñ¼¿ç]žk»¿åv"@Áç¿ïún×S9AGNfsrq3FGL J0051.0-0649PKS 0048-071?ïü¾éKð>?7ןEª?:µ ~²?7ןE§?ïüìV_
'?R$#BŸè?8M®Ïz?R$#BŸä?ïa¨&µ?Ž`Í`'F?"ÞŠû>)W?Ž`Í`'D?ïú҅x1n?4ïf?Ï]P?Dµê:HÃ?4ïf?Ï]T4FGL J0051.2-6242?Éïf‰óóÀK6W}•WÀ8¨ìëPE"À;š‡–ü@ÉI®áÂ?ùWêï̓?§ߜ]?¸'\»Aßô@¢:lãX*@hη	?ï1Çù(uj?Ðó=å=ÜÚ¿ÔæФGÈl¿Ók={5«^¿ÛýÕî´~!¿Ý̩܇ÕÍAGNbll3FGL J0051.2-62411RXS J005117.7-624154?ïýÒþÌ?,­È¡9­ð?1h—œq?,­È¡9­ä?ïõñàÈ©é?tٍ¿ü¾?T>n¬-#?tٍ¿ü¼?ï£éá}¡?‰"ñël©«?‡¸ —ã?‰"ñël©§?ïùN‹)«¦?>Sèáæa?JÅÓYQkK?>Sèáæ 4FGL J0051.5-4220?Ò'54ó'†ÀR²~|âÀ:Ju†"ÚÀ<vÀ5¯å@3"±¨Y%@rhż7S?ÂítAVâ?Ñô>Á0âK@	æb I@	sM힩y?çÃßoŠ¿å­çχ'0¿êRª\_|g¿îô±ë±¿ï5ç­ù¢ï¿íO›ÿO€òAGNfsrqPKS 0048-427?ïâxî…7¼?{|bYÍ4?m‡zÈD?{|bYÍ1?ï+åa0?¨ÛA¾ 5j?Œ:5§´*?¨ÛA¾ 5j?햃0$l{?¡M§
-Î?³Kæ~ܜ?¡M§
-Î?ïQè²H²?†ñ0ÎÎUÊ?•Þ"é¶é¼?†ñ0ÎÎUÊ4FGL J0052.9-6644?Ý)4À³òÖÀI28ÅCÀ;DʈNî{À<ô±v/@žë‹©ÁÛ@m‹Ù½v?ĹÚVÎû¿RqÔ®˜"?‹,1"Å«@d3¹jð¿ã_mži3¿Ù(À]ӚǿæøÀ$óª¿ÎïA–Î82¿â ³Ô®Bž¿ÛÖò FAGNbcuPMN J0052-6641?ïûëÚ¬4e?6Ï,Õâæà?@P•O.nx?6Ï,Õâç?ïý¦dîdŸ?Fd6"¥}?2Ì،Úþö?Fd6"¥q?ïó¶NÊL?c-Ïò–b?YʓbkeÌ?c-Ïò–aü?ïùR]€0Ú?8×åEµFð?J¶‰ÿ<•?8×åEµG4FGL J0054.4+8627¿ì«b%^£¡@7"æŸê%À:ŒAÂB/À<zxQJ@Gœ£º.å@Vº «q?Âàßÿ.žÏ?¾Þ"4³;?ô׿T>E¶@'õf?íâc¢fǵ¿äê>xâ¿ç]?`¾à¿ìiD#‰¿ïÿýaw?ïÿéÅ+ÜAGNbcuWN B0046.2+8611?ïôöͼ?]à	1ñ?VÁÖd†Q?]à	1é?ï¬úçñÇ?¥€cû±õ-?"ùÁFŽ;?¥€cû±õ.?﷙!5ˆ?€q"žýÐ?'·²üø?€q"žýÎ?ïYçì@?†ŒjrUœÌ?"Ã~—þP?†ŒjrUœÌ4FGL J0054.7-2455¿ê#óPÊxÀU놘5ŒÀ9igH
¶À;õ8Lw§×@ %"O…y?úîuÿ`Ð?±YéA¢?³¨Ö£eJ]@-J¡!@§
fÅÜÄ¿æi'z™#¿Ú¡5Ú­` ¿ÙWQ †¾¿Ö4;‹ú¿Ø¦•€…K"¿ÞAÒ½ý|AGNbll3FGL J0054.8-2455FRBA J0054-2455?ïü–ãáãˆ?4ÚÙ&	8M?;HàðãÂâ?4ÚÙ&	8;?ïûN±ø1{?_g֍'ÞR?BÅ8:e?_g֍'ÞN?ïéÇYLúŒ?kߋ÷+¾?f8¦³tI?kߋ÷+¿?ïä'ê÷×Î?_%)Ký¡·?kØ(1‡?_%)Ký¡«4FGL J0054.8-1954¿í+¶5ÝÀT¯ƒÏ,ù]À;V¢¤V§À<³6z—@·"6Æf@ÛeìÃã?Ë8àä›v?²'xÛJ?çy>@Øb@q¦KÝ«?ïú;Àu{'¿áZ³À6fn¿åôIÔ_h¿ã=ˆÁÛC¿êÃ
¬+l•¿ïàbb ´AGNbcuTXS 0052-201?ïþåA|à?1cÆQG?!«è>í?1cÆQi?ïüdýÌ?YŒmû?<Ø‹'¤2?YŒmû?ïÛg0¨Tó?u7dR8½?rLg«Õ†«?u7dR8»?ïùúŠI³?;]ðÚ(q–?H¡ÖÙ4H?;]ðÚ(q@4FGL J0055.1-1219?æ¢RÄ]kÀRʯáÚ{À9ýÜ-'àBÀ<m×ΈŽ¯@¼p¬'ð@
'¤Òh?¹ãD![ß?ÀÞÏ-Ðã@F{¢7ÍÍ@2"iY
?ïç«?´Jö¿ÝA"ßþÙ¿ã—všÙ5¿åüŸù/+¿ëC0×8`š¿ïÿÒkÀAGNbcu3FGL J0055.2-1213TXS 0052-125?ïù¨ð+–ì?F›e±W{?I\?Q¤P¦?F›e±W'?ïýÈ/]EP?L6t%ø.r?1¾…Õr?L6t%ø.b?ïO¨¤à]p?é™íQí?–
ëcôR?é™íQí?ïûšƒÔö$?3ԚR¿Ò?A•ð¬'u"?3ԚR¿Ò4FGL J0056.3-0935?Ò0Wjí9ÀÀR¸ºÇËÀ9}îþOü˜À<÷FóÚX@ù¹î"ÝÑ?ýÑ–^{¶?°_˜kòˆ?|OðŸ%?ÏÝ=ëô@÷ü\‡jm¿ë' À¿Î7¿ÓƼgyâ¿àÔÀ·Ô£¿Ú:@m®YD¿ây…'`lý¿£\»~óAGNbll3FGL J0056.3-0935TXS 0053-098?ïþ£püÒ?á'Ü«–[?%Èð2Þ`x?á'Ü«–?ïýì@zâÏ?K•«¯Î¦?0ü(éwt?K•«¯Îº?ïò:""x?g© hzž??[‹óº÷?g© hzž;?ïýwºåh?)yPÿI¼?4B/˜ÔÒ?)yPÿI|4FGL J0056.4-2118¿çñKJyÁÀUþ!ÙnœÀ9Œ Á@§À;ý˜K$Â@"żãÊ?û·ü«·©O?³+»Æû}?¿›?¡€˜Â@Œ˜¼úDz@	Ê'§…?ïÒ"4ÕË¿Á9‡ ÄÌ¿Û<á²·ù¿ÕŒò3Ž£¿áV:¿n•_¿ìcxt…äAGNbll3FGL J0056.3-2116PMN J0056-2117?ïï"Ê:>¸?`"—e'ü?`Ý5ÅÁG ?`"—e'ú?ïæÿé
?' Fýs¤¦?iòô~u?' Fýs¤¦?ïNÓ:ê‡(?…%–ɶ€?–%˜¢¯Ë?…%–ɶ?ï¦9o™e?sj7=*¢?†q¤=¦Ž?sj7=*¤4FGL J0056.5-3936¿ïÝ?¶¶ÁeÀS^/@_k À<6ë!LÀ=¬Âý@2@½}9;¶@%1ÛD^Õ?ܪâ`?ï«W½V@)x]@°Ac¢'»¿ïûvÞ®¡"?ïÿ™=SG¦¿ÄOF,Š¿ãuC
›Éö¿ïÿ¾AÏ?Øх™1"ÎAGNbcuNVSS J005620-394144?êŸÀöó¤?Æ!­¾dh?ŀÿ"$1p?Æ!­¾dh?ëwðÿÆt?Í൶B¾? <çÂ.?Í൶B¿?奡Ô'?º?C¯¦>?Õî´¼Wò?º?C¯¦>?åþîâ~‡ô?½ä{‰?Ô";ð?½ä{‰4FGL J0056.6-4452¿¹ÂNn(ÀRg ù	lÀ;/­¯ÑƒÀ<ÆuŽøUè@ˆfed³´@½ãÖÕ?Н™šäó?Çj½m^R?ò‡'Ñ(| @"'R"aª?ïþ·€ŠT¿á3A
ŒJü¿á*XÎÎ.Í¿ë)«Êô…x¿ÙccGP!¿ïÿQ"W6AGNbcuPKS 0054-451?ï÷£{Í g?T{¢¡¢6?P¹e¿1k?T{¢¡¢8?ïól4v~•?kXjÊüx=?Y'—ԓ?kXjÊüxB?îlvö}"?›tôò²×?©8˜&'Ü?›tôò²Û?ïΨÞvQ?jcÑtì£?xø+Ä×S?jcÑtì§4FGL J0056.6-5317?í3[½G5ÀOèMüãÀ:ïiÓÀ<ÔüA.žy@õPŠ\õ?ÿÖt|?Íü´Ük%h?É-´C>??ûG
‹ýá@n³}ÆTc?î9•"zœ¿á,c5Y~!¿â²Ÿúܪ¿Þts®M†¿æ̚wåê«¿ïûç6Û^`AGNbcuCRATES J005630.93-531931.5?ïþÃ!œN?'5ÝØ9£?#Íæ>#v?'5ÝØ9–?ïþG~ó‡?I½þ_ÄÍþ?+ŽhǍa?I½þ_ÄÍ÷?ïÍÓ{\?w°4¸¡Í"?yB|Ѹª?w°4¸¡Í˜?ïùÃI¨b?7".9–E?HòÙ^w£Ù?7".9–Dó4FGL J0056.8+1626?äȱÚg…ÀG5HUÚ'(À:úÀ%zÀ<ŽOÙ\'@Z%"ü|?ýÔ§Ý);c?×spºþI?ÍËù'ɝ˜?ó«¿¼CÎ@Ÿ''À1?ïԘ"¡¸¿è¸¸G¿ã3Ìý¿Õý-};¿õ¿êÐà"&þ¿ïþÈþ3:AGNbllTXS 0054+161?ïù‰8ƒÍ¿?R‰äIRÏ?IÛðÉâ?R‰äIRÊ?ïùB·ómç?_¼IíˆgJ?Jõ 2Hg]?_¼IíˆgJ?ï´	Zj]?"‡­³Ìs?ž	~Ô²´_?"‡­³Ìr?ïÏ«Ý`Z?f\½­.,Z?x*|'OÓ?f\½­.,\4FGL J0057.0+4101¿œ¥È»:e\À5×qûÅޜÀ;RÏè
?õÀ<Å ªšrÝ@ '¶%–h?þöêB(™|?ÎxADÃÔV?È#ýu·O?ö'/ðˆ"¸@²æ˜>%¿ìuŽŒö(¿ïþÂé<+?ïú½ÖÄ.¿çÖBL*Ñ¿Ñ;\øSŽ¿ïÿŸ‡ð#êAGNbcu87GB 005415.3+404404?ïüä¼}~é?8›Ø9ÏÒ?8Ú·A?8›Ø9ÏÓ?ïþ:r¤¾Ä?PàME)O?,XÕ´Á"?PàME)P?ïœn^Ùé§?…vy¡B?ˆähI…–j?…vy¡@?ïóF7¼Á?OWÿç4f?Ys†}Ð|?OWÿç4f§4FGL J0057.3+2216?ã;e|!'ÀDIúÁҝÇÀ;®ÈÕÇGÀ<¥h[3,@¬ñ\y'´@G•övêB?Ђ§z,ìÈ?ˑb"së?øŽv pMp@‹ND†˜?ç{âN"8¿Ñ!Åâø³0¿ÛK·c"ä¿æ#ª"" [¿çñž¨ÍD¿ïøuÈ9pAGNbcu87GB 005452.5+220227?ïÙµQ¿"?rÕ>Nx?s{¥W 6?rÕ>N{?ïúÔäŠP?[È/~w?D¬mÖ¿½O?[È/~w?îàm¸b›?•‹l/šd˜?¡ù$x	ÖZ?•‹l/šd˜?ï¹E!d?hO^áÀÇ.?®·º¹fë?hO^áÀÇ.4FGL J0057.7+3023?Ü­eÄ;À@:2 f<uÀ:]á‰ó3iÀ<qƲ˜¬@à[À6ã@/¿üñý?ºW¬5Ów¿ù/£©	q?áájžYqá@h…2`z?ïÞßY—K¿ÚßùD¤õ˜¿ç2Ö·1Z¿â·U¼®¿å"÷¡aº¿ì\8åú›<AGNrdgNGC 315?ïßì†%i?g  ;w‹?p‰¼íJ{?g  ;w'?ïôDß³"?p)"­ÏV?WwÒ@˜ö?p)"­ÏW?ïzæ8F«?‰vh†o6?£8÷*Ÿ¤?‰vh†o-?ï°µ€mJ?jçGùËÙ?ƒÒœä­ä?jçGùËß4FGL J0058.0-0539¿ÆÉ'
ÕCÀQ1&éyÀ9àL'ÿzÀ<>$ìz@Ž¶çˆ:@Œ_|gY«?µ¹f"‡Ý?š%™¼Úç?å·;"@ßÅÍÕ¿¼o¿*¢Àà¿äu0cu^¿çéâ‡I5¿àïâEÚÕ¤¿ð?ïÿÿ" 5•AGNfsrq3FGL J0057.9-0542PKS 0055-059?ïþäR\? 'vöì\?!ºÞ¯š3¥? 'vöì{?ïþ^iU?Az½3‹_¯?'*oŠ ?Az½3‹_©?ïØ4aM:?zÏ– ݁?såÏqÙc?zÏ– Ýu?ïÿIÿžt²?÷·\|?À1i°ú?÷·\|\4FGL J0058.0-3233?앒Ð…«ÀU>úç'À9?ÊKM
À;ý±Ù+á@›4
MÆ\?þ§"Ô@^•?±MŸ^ï=?ÃüiÈp@ÒàýÜ9Q@Ãö9'­š?Ì♨28·¿ÚtØdZ…¿ß´© !óñ¿â—¤—#"¿å_‡dU¿ídÂw^[AGNbll3FGL J0058.0-3233PKS 0055-328?ïΟNÅZ>?wcÿЫx?x°XRà™?wcÿЫy?ïè'-p«j?Š•]™)?gØҏT––?Š•]™*?îð¤ˆþބ?™!ƒˆ? õ·pÖ?™!ƒˆ?ïÆ´Â|à ?m*%éÊ܍?|¥žÁðr?m*%éÊ܊4FGL J0058.3+1723?í‰ëøa‰ÀF¹àÞ҈ÎÀ;ײˆä@À<àòŠÌw<@"\øžC"?ö¬ôI:Ü?ÙWM¤xšÆ?ҏ4¹¿ª?ûG&Ɖ½@1ƒ°¤"¿ÎЈgB.¿ï¼ÚF2y?ÄO{τ7?ÛbY&D¿ÕäŒq'êS¿Ó]$É8AGNbllRX J00582+1723?ïùBДÖ?D'füÚ?KŽô½¬­^?D'füÚ?ïý3¿d?QKæÿ+×?7W>bъ?QKæÿ+Õ?ïÑGHF?wCL§ŠNæ?w\[Àvܺ?wCL§ŠNØ?ïö
ðÂ-?M`Ԉ$£?Säð{¥Î?M`Ԉ$•4FGL J0058.4+3315?ßóTïŽ=rÀ=™-ÛÛ]‰À:ŸZ±&~À<ƒ3ÆÖé†@¬nëÆ>@iød*L?Ťò}¶d+? zƒB®êþ?Ö¤b‰·ú@M™»ÓU¿ÚWvÿÄ^¿êxbý¦3†¿Ü›aÅ¿ã½#â]¿æÖ©ZýV¿ïÿ¼ä!}(AGNfsrq3FGL J0058.3+3315MG3 J005830+3311?ïÿ5*g­[?™ÿöñÀÆ?Z³
T˜`?™ÿöñÀ¡?ïþǃÿÍè?H*™‹CZˆ?#‡À!Œ¬?H*™‹CZš?ïݎbi2?wù*¬Õ?q8ÎôËg2?wù*¬Õy?ïÿԕ|
‰>êò
ØÛ#†>õµAú»2>êò
ØÛ#®4FGL J0058.6-1140¿èÊ5ùÕR`ÀRiÂ;ySÀ;Tük 	‹À<¶g÷`N@¡'ðµµ.@Êyžø?Äqw¼zL¿£ð ¢³"ã?۝i?þÁ¶é¶'y?ï¹c<{¿ç³ì+7¿ËÑþdõM¿èõ¿Ÿ½ 	¿ÕAé"h"ú¿ßÒ=ºu²4AGNbcuNVSS J005832-114050?ïùŽpyD/?Eþá@¹f?IÆ>ïG=?Eþá@¹f?ïù²ûÏCÎ?a¥ÛLþ"?I4Âðͱ?a¥ÛLþŠ?ïÒqc=?wòœµ`Ô?výGwNaÓ?wòœµ`ß?ïðxï6A?PŒÑ›kD<?^ý!"}Û?PŒÑ›kD64FGL J0059.2+0006?«žØu‰†¯ÀOXn¹ªÀ:Ôf_°iÀÀ<g[±×~@ðü@\†Ô?Æ3°†›;?!ßÑa\w?•GÒ¸°Fk@Ê}ª{¿ïûSþ"Õ½?ï"'úñ¿èýk@íù¿Üo<"ððÿàÄŠ]¼t¿ïÿ·¼]êAGNfsrq3FGL J0059.6+0003PKS 0056-00?ïú¢g¶Xz?J*}ù\)?Eva&žW?J*}ù\K?ïúñ",`1?dÌ]¸(?D9¯N;#?dÌ]¸(?ïn›—ººŠ?ŽC¦ãÎ?',¨®È?ŽC¦ãÊ?ï÷gMV¸ù?Cƒ0Fûä?Q1eRŽ!?Cƒ0FûÁ4FGL J0059.3-0152¿Ôÿ§¶çÀP+±mÀ: ö|ÉÀ<om"BJ'@!1‹¾9·?úJ"H)d}?ÉT™_b@?À:îéWG?öäŒ×ê7@w¤!¸?ïNëUN.¿Úb/ »è¿ëM&ßgÚ?Ù>&@Üi"¿Þ‡j'̔¿âqÐý³õeAGNbll3FGL J0059.2-0152RX J0059.3-0150?ï÷ÍxB*õ?TNí´""?Pe{ªQ?TNí´" ?ïûf¸–_E?TéP
sþ?Be¦'ó$?TéP
s÷?ïÁԅŽ(?'h'¨b?w½8ë7?'h'¨e?ïåS
†"Í?_(X;õ1ª?j¬õyk2ô?_(X;õ1·4FGL J0059.5-3512¿åÄHwÈhÈÀTnñVIÀ;-‡˜æsÀ<×hL´@ '¡R Œ?øàLÜQ¥?ÔÓ)=+Ç?Ú·æ@'?®@ºQÎ_@'.¦[žâ?Þ÷~°4;¿äRKý."h¿Çáä÷eý‹¿ÕÝmCzS-¿à_'¡Û\ˆ¿ïüjÿÓ4pAGNbll1RXS J005932.3-351049?ïøXséY/?M½'‡¼—Ã?Nž0Z›H~?M½'‡¼—Æ?ïüŠ
ÄQ+?RٌYS]?;¯'Ýv²?RٌYS[?ï›>CÕ?‡þl=µ%M?‰:0o
»þ?‡þl=µ%I?ïÜ'	#·U?c¾rw_Â?qì{n$Vl?c¾rw_¾4FGL J0059.5-3338?éþ¢·…
¿ÀTÐwpyåŸÀ:îßDž•'À<}þæ$Œ§@ÀQ>@s³{j?Ä(3e]&ø¿Jèåë‰?Å|ÔýGéÏ@8WÁÝÛ?ï€wSôsÛ¿çՊv'•¿éÈ	ïm¿å
@Zc"å¿îâæů¢¿íå¿ý±q'AGNfsrqPKS B0057-338?ïúdxÁû?HñçõáÕ©?Fnûø?Hñçõá՝?ïåJV%Ô?€ú/T"Ä?jµ©Úý+à?€ú/T"Ä?ïÒ'ԕp6?w™ÿ-E2Ñ?vìµGåI?w™ÿ-E2Ô?ïòw¦³GP?LƒCr«&?[²™q_˜?LƒCr«%4FGL J0100.3+0745?Û&™ž­ÓÀK…}™ˆÓÀ9À~à°¯À;¸ ؽ›×@~DzƒSÝ?úñ`åóå@?°'IïgÂ?Ãahz½¶Y@Y…ðoiD@
õöA:\ó?ïãqߖS¿¼j»_¼þù¿Ôþwštá¿Øót ¹3¿áÏû'½¿ëÝ­Å ‰AGNbll3FGL J0100.2+0745GB6 J0100+0745?ï€ì½£-?ˆ/u0:?ÄЗ4¾–?ˆ/u0:?ï¡iÂr?!?¦‰ÊÂh;?‡¥cp7¨?¦‰ÊÂh;?î×ƒ¼Ý?œc`·|ò?¢7Ä2.?œc`·|ó?ïŸMD3©?‰ŒÊµ¡äH?ŸÌWyŠÌ?‰ŒÊµ¡äI4FGL J0101.0-0059¿íûÍ¡{ÀOáXâe,À:봙Р>À<[‹)"N@•)œ±|@mFTx'?Çö¬m±´¿"o:Æy³?¿D"Wá@àG
€Œ'?ïQSµø ¿ìŠ…à)Jý¿âÛȳb˜|¿ß㲁òÞÚ¿çï\¿Hª¿¿ïþÛ<ÒfAGNbllNVSS J010058-005547?ïû:;ó?B™Š²'tØ?CçÜ4v?B™Š²'tÁ?ïü"‹@ó?Xì—E·ß'??[¥øeÉ?Xì—E·ß‡?ïȌ­dPÉ?}ùYå»ó"?{¹©MכY?}ùYå»ó'?ïõ‡&~K?Cá\+ÆÏ?Tñ²ýkõ?Cá\+ÆÃ4FGL J0101.7-5455¿Ñ5G¾1ñÀOÅ?9ѳÀ;»¸¤÷›­À<ùÓ5@"CS/ÒÖ|?öÔxwàâ.?×?=ba(?Ér0‰Š­Ã?õ©óƒðºé?ùÎ
"Ñ¿ïì'œ<Œ?ïûÌ>²mP¿ä#%  ?͗J	
šÈ¿âê¦gv¿±X•~̺AGNbcuMRSS 151-121576?ïüÛI]¢Á?2ãÂ]>á_?9%µéõÁ?2ãÂ]>áŠ?ïé:)!|?e±žüiW?fÅüÖރn?e±žüiW?ÔEÔ½?…¥&²Uº?‡ÊîŠÐŒ?…¥&²U»?ïÅs<Žz?s-
Ë«Ñ?}Faú8Ã\?s-
Ë«Ò4FGL J0101.8-7543?ì^ˆ!¨P©ÀD°p~]À:øóºw_³À<drû ï@ú}µ'@'°¤xí?Æ0A¦¾p>¿©cKn?ÞÂ
y?ý$2³=Û¿è,ÊRŸ	¿ä œiàn¿êÙCӔg¿ç"\¾që*¿ïôL¾´ ?ïÀÃþ¬CAGNfsrqPKS 0101-76?ïüòmŽV?Bõ74͈?8l""Rò?Bõ74Í°?ï*ä]?Š#±F(?ˆµ~Føè»?Š#±F(?ïŠÿìÈ ??ˆ%´y†µ?@Í÷ð?ˆ%´y†¸?ïÚ
¦‡L?gŸJÙxÞj?rú¬¼YüË?gŸJÙxÞq4FGL J0102.0+1639?⎯;J ÃÀGRv‰ÊÀ;IÍ©kŸÀ<–=u¬T‡@' 'àð@P'Û_6Ç?җýãA?ÊY ãOp?óñIÈ î@ÛR¼ev|?î¥k¼½¿é"c!7ˆ-¿×»d$lÆӿ代yí+è¿ÚÒ¶Ù ¿ðAGNbcuTXS 0059+163?ïû/?A^%TÓ?C‹ÿCó©(?A^%Të?ïüÕ|Ãì×?PôÿáfÔ?9Tà™Iú?PôÿáfÜ?ïoºGW™?‹.áþ"}?'·Ýø?‹.áþ"}?ïìéš
,M?Qç&«Äé>?ceòÓ²š?Qç&«ÄéH4FGL J0102.4+4214?ë gOö¼À4–™Øƒº4À9°²2í"À<Nõw/@îȎ¤ž@û–¼o‡w?´æ&eŠ@?ÃÒr¾Žpœ@'3cښì@¨§óúc3?ìPSà뾿å¸Â>SwÌ¿êiˆ†a¿èÏ{5U¿ç'kë
¥u¿ï÷§pò±AGNfsrq3FGL J0102.3+4217GB6 J0102+4214?ïüí÷M	¼?7,fù¼O3?8E—²Ò?7,fù¼OE?ïü^3èÓ%?Y
À?=`¹fÔ=?Y
À?ïJ9¦ˆLã?pâV^&@?–¸Ë.öcž?pâV^&E?ïü	ŽË™?.ý-_eq'??³‰£7 5?.ý-_eqy4FGL J0102.4+0942¿Ê¶¿$?
dÀJˆÝ½µØ•À:áüëx‰À<i
fL@ Ά5•8?ûþ·Ë³È?ÒO)~(¤å?Âå+é<ïõ?íúö -G@ãñ@J¿ïêÜ0?ï>ž¡@¿êáz~vR˜¿ºÍ¹†ÉÞ0¿çł Ù©Õ?vCA"jïsAGNbll3FGL J0102.1+09432MASS J01021713+0944098?ïýe§Ò€®?@~^°V ¾?4ÒÁkú‹ë?@~^°V Ê?ïüRb£?TPò [Ö?=lïÒç\Œ?TPò [Ò?ïtaWÓ¶?Ódµø02?'}óÕ‰	?Ódµø00?ïí&²0Á?WÉ´H ªè?bÙMÏ>æû?WÉ´H ªè4FGL J0102.6-5639¿ÉÕRWÀrQÀN3ք³žÀ;¹¯¹–À<¥}xÑ¢õ@ 9†˜*?ÿ›øԒ"ì?ËÞs'êÕ¡?¾Üö êAŽ?îÞx@ƒ}Î@˜ªøè?îÄ8ÿzôé¿ã×ÓÐw¿Þ'•ðŠ¿äþ£%3–¿Ù߈'3™‹¿æ›Ãu56CAGNbcuPKS 0100-568?ïýê4ñ'?.ëëMH‡?0®_(st?.ëëMHÂu?ïþpFê?B"m…Øè?(þ+˜dN?B"m…Øâ?ïîy"Þøì?i!sÓi".?a†k!}?i!sÓi"6?ïò›J­ò‰?J}ÈDþ?ZÉj¤ïK?J}ÈDþ4FGL J0102.7-2001?ãòR3Ù{ÀTœWS£ìÀ;öÚó=À<ë…à1@"m.B]ž?ìHBŽðÉ+?è?àáVÈ?åÁ=¢wä"@¹`ß=è™@f±?R¦@?ìü辚Úâ?ïšÜ?0—x?® Æßwõ/?€3
.ÍÙù?Ɵ­¯Ñƒ¿äè/(âwYAGNbcuPMN J0102-2001?ïÐÒ8,"Ü?s)_6'Æm?w–ã齑Í?s)_6'Æp?ïúRÏq3Q?p`Ž:ú
'?F´Â;2¸W?p`Ž:ú
?ï"Â3!¨^?ˆ¸¼6zY?ŽÏs7•è?ˆ¸¼6zX?ïöô/ü-¢?RBOô?R ¤½o?RBOé4FGL J0102.8+5824?ÔÕ$qáT)À·ê¢ ©XÀ7Ü.u^PîÀ;GŽd²1@@6†@¾‰Þ:³Z?—?úØÍ?°©G¢'@4XÍ!@ÅéôZ/¿¾ÖK¦œŒ¿Þóc9‹<	¿ä->\\!i¿äpˆÿ¢´¿årðR
¿è(ê¿üÚ²AGNfsrq3FGL J0102.8+5825TXS 0059+581?ïýFœC˜Ð?-_¾lŽuÊ?5Ëã9}‹?-_¾lŽuü?ïùŠ5kT#?emžRc¿¨?I×*R¯u«?emžRc¿ª?ïÀf˜Æ?ƒ-W×á²?û̳·œ×?ƒ-W×á©?ïÿÀ]Íü->öY#ª7>ÿÑép>öY#ª5¤4FGL J0103.1+4954?æ)³ðÔÊÀ)ÖV%¦'¶À:o¬)ÜrÀ<
(¼·«Ó@M"àú+@Ä>š4?ÆíG@±K?¶zPÑæ?ìàÛwŠ{@×o?t¿Î£ –x|é¿äœG(³}p¿é½Ê›š$Ú¿æö#l¿êCá9Ñ]¿ïþ{€©Þ‹AGNbcuGB6 J0103+4959?ïËCâ^øi?|ç_	Š˜È?z^ЃÊå?|ç_	Š˜Ç?ï»üZÉÂ?"…T,¬?é|
•?"…T,¬?îâ
g¨Sd?–V	míc?¡ßY…zÉÂ?–V	míc?ï|¼£»¥?y‡ºÆ"î)?hkˆ‹]½?y‡ºÆ"î-4FGL J0103.5+1526?ywÇÙìÑÀG«ò<ÈÞÀ:ëCø}T¿À<^1
¿@å´ã¡ûh@ʘÅ^C'?Äé)yËóß?œQö†žY?ÕõèúÕÉ¡?õ­:mº¾¿ïûœÞÈwÓ?ïÍ$Á*'5¿åÞ¿þÞ÷¿ìÄ9ë´¡¿×ãJ<º?¼ŠC:gZAGNbllTXS 0100+151?ïó-Ï?â?Y±wVû?Yý¤a€;í?Y±wVû?ïÈLWþcÃ?Å˜Œ~g‹?{ÙÔÎl?Å˜Œ~g‹?ïB©Rv?"šåÄRÓ?œ7ªÕ¿Ñ>?"šåÄRÔ?ï‹ZÜeSi?€(Ãn~H¦?)Hæ«%k?€(Ãn~H¨4FGL J0103.5+5337?ãm!Z£äºÀ"gòä¼®À9¼ñÈ.Ø[À<!ƒÞFr@ y:æ/õ;?ú	»…|¬#?µ÷ÝòŽþ5?½³ÃçJý@ƒZ'ó@Þ¿¾qj¿ð?ð?عÚÂ-âf¿Ø("C2¶¿Ü¾ƒžZž‡¿Ú(ÔɎÕAGNbll3FGL J0103.4+5336RX J0103.3+5337?ïÿIú·À|?PÇé£-ð?À©ðŸQ?PÇé£-—?ïö&}XØ?r…ûŨ&?S³NOé·?r…ûŨ&	?ïÊËÜf¿¦?}‡Ýÿ']é?zšÌ ,%?}‡Ýÿ']ù?ïã×Ì¥<?\ý¾§†˜?lç(3ZÄ	?\ý¾§†©4FGL J0103.8+1321¿ÕîÄyûgÀH³ïàÎ'À: ù™´qŒÀ<‡ú'+6@ùOH<¯´?þê»m(ø?ËBq¿ŠïÞ?»šÚ¡Ì˜õ?ðÖáù"»¼@³!€nÅ¿Ù"K"bа¿ÓŒIåQS¿à*;½ÆI¦¿ØrÁžEzÞ¿åSUèiáE¿âæqqAGNbll3FGL J0103.7+1323NVSS J010345+132346?ïÿygñSK?ƒn\‰r?ÓՖ€j?ƒn\‡E?ïþÚN²\ã?BE¿"j'D?"[Ú1Ñ}?BE¿"j'F?ïõ©õ¶Z?c¶Œ4é?T¬"LÞ?c¶Œ4ó?ïþ²~ºM?i‰z–g?$Ø[.u•?i‰z–œÄ4FGL J0104.8-2416?秮%g%'ÀUv<òϕÕÀ9î
^u×À<|ŒbyqÜ@HÇ nM@>Vð†?·‰áÚiÝ?º!²¾iîÂ?ûúÊ8Ö@ Î|O[Þ?æÇ¢u‹G¿ã¬ ‡t~¿èÉ—ïun¿é£J‡ãŽ°¿äæZb!2U¿ïÿÕ7ÕYcAGNfsrq3FGL J0105.1-2415PKS 0102-245?ïâ«Ì¤$?®S‡–@0i?mT3[üÛr?®S‡–@0j?ïý¤E†#l?Q/È«çÇ?2ÝÓÎ䭗?Q/È«çÞ?ïÚ³}­/~?lðàÛk¶?r¦A)h@º?lðàÛk¨?ïþ˜¢
±»?Ží·í«}?&uß$ä2?Ží·í«ƒ4FGL J0105.1+3929?!o–À7Lq²•êÀ9åق½µÀ<m›2öÍ@ó	WA°O@ß^Ö?¶2«M÷?´ëÿ—û3è?üÅ,ÅZé@‹&NÉ;É?éRøàÑçi¿æÈ8–¿ã:âŠú¿âŒ™ÖÖ;¿ìæÍߜ]C¿ÜC!þ,–6AGNbll3FGL J0105.3+3928GB6 J0105+3928?ïý*B†âj?2à_ل¿?6­ëÈì±Z?2à_لÁ?ïþ,.É?G도QÙþ?/þÍ=sõ?G도QÙü?Î
Æ?‡¦Ï¿­–Z?Š{Ì}N³?‡¦Ï¿­–V?ïüü6öï?(Ò¥ü?þ?8O H~G?(Ò¥ü?ö4FGL J0106.9-4832?éà:Óï•ÀQsWæpãÀ;råx+‹À<îã>ÿP@+Ç¸æ¼@±¦»ÁÎ?ÉW_ã?ó¿³ÍØ®?ã,Àþ7~@¼È}‡À(¿ë­AJÅ¿èpúß.Ï ¿Úò yI¿àIÏâ€é¿ïÿ¶.$Öy?ïü¯ž=Ã/AGNbcuPMN J0106-4831?ïô¯;ç¥?aœëz³?V¡‰Ü0¶´?aœëzº?ïðÀ{x³?xP¡Y¨«?^~ý	™€?xP¡Y¨©?ï\cà
Ä}?$7I»ÊW?"sƒþGpK?$7I»ÊV?ïùÐ߈?A5‹Õ¡À?Hñ¼ßåž?A5‹Õ¡À¢4FGL J0107.3-1210?ëM2èí\­ÀR¦JŒL˜À:ºœiànÀ<ŽO'…€@ãg_ƒH@8>ž¡?ß­¯Ñƒ?¶ÊÿB?ë}?ó>~:˜'B@F
ú"†4?×·IbŸ‡o¿ß@zC'ý¿ç*
Osۚ¿á}¸èi¿ëÆÏ\Ê¿º¥@v'AGNbcu3FGL J0107.0-1208PMN J0107-1211?ï÷dÍü5h?I¸×&H[;?Q6d•0¼?I¸×&H['?ïúwQŸš?^Å1³;Ì>?Gš"¹žh?^Å1³;Ì>?ïÊÂ
H5?€ò›†mTQ?zžù[·åš?€ò›†mTR?ïòÔËÎ*H?IB4'îBÕ?ZVhc«nq?IB4'îBÕ4FGL J0107.4+0334?Ô<Ôÿ›©BÀM‡æÕw–À:ˇõ,ggÀ<_"žy_@½$x°?ù@chºÔ|Ä?Äs¨è茿¬/ñ¤|O?â³Jå×_Î@Rú_W(†?ï–ÄÓG³¿â^•ýWÚ¿äæAGÈìm¿äpý÷<7¿Ös©Ïr¿ïÿò> wAGNbllPMN J0107+0333?ïþՈÆn?¬q'ÙÞn?"§s™ »?¬q'ÙÞô?ïþáù©¼Ž?<©ýì
O?!àed7?<©ýì
L?ïçöK€ >?o=%8…?h	´ßÁ?o=%8u?ïþҙcWš?®‡3;–?"ÖiʆWÊ?®‡3;–>4FGL J0108.1-0039?î՝þFÔÀO_ïIÏÀ:;+@ªÀÀ<}7%@'/m@§'…€Þ?Ä °¤£
?·p²o©[.?ñƒSV¿)v@Ph$»¿àd¤à¹)¿å[ÃÀ^ªZ¿è{.¿±q¿å¥ŠžT~¿ïÿªoª²Ç?¢''%ߍšAGNfsrq3FGL J0108.5-0035PKS 0105-008?ïñ\-f`$?mÞó…Ö?]G¥3?¸¯?mÞó…à?ïÆYA碶?Œ£w/?|Ó_.¤Ó?Œ£w.?ï=%SëÐ?ÿ´‹?˜[U'…ÿ!?ÿ´‹?ï¬W°ÌÕ?tº¼e2w?"êÌÿŠ¼?tº¼e2y4FGL J0108.6+0134?ïÔl+6HñÀN~ß?–À6ÉÁö¯õ&À;)׆d2¯@ìPGk#@FtÃ÷;5?†j½ýÀÏW?º²ËCàª@-ùmL3µ9@!‰q S²…¿ËÅaž€‰¿áÆ,¿Ñ'®¿åû"y™¿æPÕÛiH¿êk¹AT´¿î¤;I'*AGNfsrq3FGL J0108.7+01344C +01.02?ïó€f9".?UÛgyRÐw?Xÿ3ŒÙ¢??UÛgyRÐo?î÷/¦z~?¼odJ©\? ˜X†?¼odJ©\?ïځE†e?•&úžÛ?œD¯×O3c?•&úžÛ?îU%`ÓZ´?¬U%¾ÉÎÎ?ª­©òÊT£?¬U%¾ÉÎÏ4FGL J0109.1+1815¿ïý!ì€mÀF3¬ÿiÀ9'Úa
À<8.j€@q©(ؼ@cH¿Œrj?²µ÷‹'?¯Èî_³]ª?û'{Gžû@?Ï y¿ÜÜCB	[¿á®†ü#»¿ÜÎÊ}è
E¿áäÃßt¢¿á>yî§z¿ìþ3!?•ÂAGNbll3FGL J0109.1+1816MG1 J010908+1816?ïÔ5zNí?pI‰Ê
@u?uåBØö‰(?pI‰Ê
@r?ïß¡AÞôÆ?"{õC΍?p/_…?"{õC΍?ï_½Ð¼¯?|×TúŠ?"EèjÆ?|×TúŠ?ï7˜*ýµk?†l0#žÎ+?™ú IRŸ?†l0#žÎ+4FGL J0109.3+2401¿é©ZõØ%ÔÀCUGNΚÀ;¼|óp¦À<xwiÃèø@X.8¢ˆÖ@ç¹Å‰­?Ǭ0,–¿Ÿ"|Ái
Ø?ÕZ@ÿÚÁ@‹›˜w?Û¯ç#e4ã?ãeC»¿ê$kºc=½¿Ê[ê·nkÿâ["ötf¿ïÃ;ã?ÖAGNbcuGB6 J0109+2400?ïû6zK¸?C'Æ$‹Ò?Cç&Ñ"?C'Æ$‹é?ïþnãίæ?I_X@³Gø?)ê5?I_X@³Gâ?ïÚî5høb?w¨7äDƒ?rˆåKƒÏ|?w¨7äD†?ïüÌY7X?29h:C"õ??A6E9s?29h:C"Ú4FGL J0109.7+6133?ëJw¶Wî¿ó¸SH|p"À8-Ðé'ÿqÀ;áÝÖ	Œ@"ÑéÂ&@""ãw3=?¥,È
`)?Ä=2»i"-@–6mzVÞ@hZm߬x¿ºÅM~¸î¿áœ§ê9¿ç΀2ÀG¿éokþUÛÕ¿í²˝!ä¿ïÿŲýîAGNfsrq3FGL J0109.8+6132TXS 0106+612?ïÛ¶¨u¤¨?r_è~ò?r$«Å-«†?r_è~ð?ï³â
ý@å?²BÞzÎà?ƒ|€¯Æ"?²BÞzÎá?íÀ©pèÃ?¥R:úÎd?±ú´ȹæ?¥R:úÎe?ïñV'/ä?PUA>ãì?]Rû¡ú9h?PUA>ãæ4FGL J0110.0-4019?×5÷g	9ÀS™Ì¢ÛÀ:õ"£Ö3À<­9©nù³@ ›èÔ?]?û!³Éƈ?Æ	E£ù?ÀüÆ$<k?ú÷YhQ"@¹ˆºa¿ïÿ¬=`2Æ?ïí«3õÐÒ¿Àµm ‹]¿ÜϞƒŽ?s¿èU²Ÿ$?ÑÝсèMAGNbll3FGL J0109.9-4020RBS 0158?ïþ«Üé?3*Oû³a?/ÿ5B1z÷?3*Oû³~?ïýñ#$[?EØT‰,?0væß5+{?EØT‰%?ïÆ7Ð
<x?}ù¡D.µR?|äùaÄ|?}ù¡D.µQ?ïö7B0Ü?MWٙ{ŽÒ?S'{žG¾?MWٙ{Žð4FGL J0110.1+6805?áàÀ¬æWÝ@(X¡ÅgÀ8qö_mMáÀ;¥Ý·Ö›ƒ@ %jvÁRp?ÿʘû(¸?¢6ÿ#>Ò?¶n]øû÷?à¡s†Ž$@qÓ%V{¸?ïßÑ÷®ø¦¿ßA–bØg`¿âýÝÄ쯿ݤÙÿj+¿Þ…"/_i¿ÞJ™¡|<AGNbll3FGL J0110.2+68064C +67.04?ïèÀ¦\?goƒ%Óª?gã?âY£«?goƒ%Ó©?ﺠ¬}ßf?¡Ú¦'ºh?WÔàˆ&?¡Ú¦'ºh?ï$
ÏÙ?˜.fu'nŽ?›~½Æßµ?˜.fu'n?îÌôQÛ-X?'•>[Ë­'?£0ºâM*{?'•>[Ë­&4FGL J0110.2+4151?àöôAÀ4à@žUÀýÀ;¦ºq€uÜÀ<Ðà`'ˆ@"±ñ°Ü×1?úH­ž3\N?˚R¼iš?'òk—Ó›É?ʉ8x[@¦èxyä¿ïÈ8}õÏ%?ès5Â¿æi
_¹ùá¿ÅJâ&{>æ¿Ï&ż9¿Ò;lˆÌÃAGNbll6C B010709.9+413321?ïÿxn[é‡?yœ	o?ò4'ÏQ?yœ	o?ïþ´³¦fw?E3¶"ïn?$´Å™˜•@?E3¶"ï[?ïëîÍÒØ!?oÖßa-ûª?d2-'ތ?oÖßa-ûµ?ïþ3üh6"?"âЄ
"±?,À9|–å=?"âЄ
"<4FGL J0110.7-1254¿ï—~à[<3ÀRÄéÌ·ÔÀ:¾šþ§±À<Š®ª¢ÖY@½iLʳî@Pys‡?¼p1v´½¿–û^c@J?ÞÔâÛVþ?@9ä>-,?ïÿQ÷GË?ãÙª*áU¿æp·'¨å¿ê\Ïä¯B?µ¦ï|¥¿´Af|¶´ÝAGNbll3FGL J0110.9-12541RXS J011050.0-125455?ïúWâàÌ?HF¨Ñña?F täÔ²?HF¨Ññz?ïü¥K¦?LäQg
¼'?:Õ§B̚?LäQg
¼ˆ?]7Ez?‡ø‹Nä:?Ý¨².¡Ø?‡ø‹Nä9?ïï5l©?V¥¦1c?`Êbû"X^?V¥¦1`4FGL J0110.9+4344?ᵊ;ô%À2ûÕýÍö˜À:Þc'í"ÓÀ<Šj}L[ù@"'ÌñŠÇ@á߃ˆ¶?Á1¨r¥d?vëþà(è?½ªñ°±ä@Uuów0Ž¿'…ÅYïh6?ת#Õr8¿éâ6Ó¿é ž9$å?Å~{
ã3¿èŠ= ÿ:AGNbcuGB6 J0110+4345?ï÷qd›s?Rè×vÍ©?QË6É?Rè×vÍ©~?ïþ¤qºòâ?Nk²ý–M?%¸äPÑë6?Nk²ý–=?ï´šxw?'l¦à	L?'ü8aáÚ?'l¦à	L?ïþ…RƒŒt?.¨1Ú?'ª×Ç8Õj?.¨2G4FGL J0111.4+0534?ïºB_ê÷¹ÀLxYÈÉ2À;r.´ƒ*À<À±Ù+€@ Øp±?ýñ´âg?Òص8[' ?Á8CyT?í6ͼ¶Õ@p]i!­¿îù/Lñ ?ïý°šgó¿èÆvÁþ<±?±e'«é¨P¿é.&ïX¿Ìò¦%C1AGNbll3FGL J0111.5+05351RXS J011130.5+053612?ïþ¼e•Ä¨?*o.!w{c?$9¦£µq´?*o.!w{{?ïý6»•?L뢖	 É?6K'#T?L뢖	 »?ï•mvGޑ?‹Ókõ^:?Š¤¢n[Î?‹Ókõ^9?ïøcG
ÆÁ?Eºe2k|w?NrãÔäú—?Eºe2k|w4FGL J0111.5-2546¿ë­Û.‰$ÀUR¾7ޓŸÀ;0÷b¢Œ‡À<¶53¾sn@C¤Ýšzj@'Ýãu†?ڊVwÜ?È žE¥Ñ‹?íÓõƒ¥@	Óf'Ò,¿í!*¢jùs¿àÈ3?Èlì¿ä^1¾éà.¿áp—AЄè¿ïü楻æË¿ïdÑ`…PâAGNbcuNVSS J011130-254531?ïþ׈ò?-þ£"Ùrx?"ƒ×°áž?-þ£"Ùrå?ïþf×w»Ø?F/|=/%?)'ˆ"B"·?F/|=/?ïY ‡ô?Œ»ö21ï|?"ËïÿÏ?Œ»ö21ï?ïýÂFâƒ?,Ϝ¤'®ï?3íÈëê.?,Ϝ¤'®Ö4FGL J0112.0-6634¿Óƒ·+GyÀI6<tûT À:S@FA,ñÀ<•Ór²@ߟ²ãA®@gFÂú?¼˜ðý-½¨?¾
iõçù#?ýŸ¼ÉIŠŽ@	š"‡0áI?ϓ˜8E–¸¿è÷̊‡­ß¿æf'Ï ¼¤¿ìj`%څ¿åÁ/ÀbY¿ïöm_~ë˜AGNfsrqPKS 0110-668?ïþ½^ã*q?"x
Þ®?$*ÍXèà?"x
Þ?ïûSÀ5Š!?[›2vø–?B°ÿ)׀F?[›2vøŠ?ïÜΠá_?o;´d'`b?qõ¯Q?o;´d'`X?ïâ#¿´îã?\y0&8·å?mÜ@KC?\y0&8·ð4FGL J0112.1+2245¿î$¡
€¢XÀCïmÁ¤zžÀ7MØYÈÉ2À;%IfË@'P¹+@¼Ú'.?'/,¾O¢?­:­a2Ü@.&,ƒí@2od;黿"ZUû£é˜¿ÝŸâˆö´'¿á›žV—¼J¿á1xþ™x¿ãò«G£¿çåøL­W¼AGNBLL3FGL J0112.1+2245S2 0109+22?ïøã¿sÀ?J‹'cŒW#?LqÞ1D?J‹'cŒW
?ïð›°"E?p.p|8*?^ȟݻw3?p.p|8*?ï½
Ý+Vé?"ÈÇå
n?€¼ˆµ*E×?"ÈÇå
n?ïñ`þ&l?Q‡I±"k?]>Á³)h?Q‡I±"u4FGL J0112.1-0321¿ìK¤2•­jÀPnk΅3±À:MÞÌ©'^À<YÙAOU©@sLYŸÙz@Öðd‰Ø?ÁË©â,£?ÂÞt"ýS?ýJð
­@IV‹'?훀#¦Î6¿æþ*¿æèɂ•q¿ê¯ ²¿â¦=Kºéu¿ïÿT©¥€XAGNfsrqTXS 0110-037?ïûVœS+?CC@o?B§¡Ž³W?CC@os?ïù»ûý­A?k"؉ qü?I	JþÑ?k"؉ qÿ?ïÊ8v@¢?v×b‡.¶§?zãöD߯?v×b‡.¶ª?ïÙ$y®]?b™ÅßDá?smÃ(ÑrS?b™ÅßDß4FGL J0112.6-3158¿ïÂõù<NñÀTÓü;OagÀ;®¬A<
rÀ<õË^7ü@ m®@o±¿?ö
þ`Ï?ß]àÛÍq?ç\3rSÎ@"ìck	c@ÃüÏHýö?ê³rôb³¿ïÝHæ"ß(?ìM¤=Œ}|?¹–@bŠ~¿áÒ¨ëÎE¿ïùêqùA AGNbllRX J011232.8-320140?ïäêJr?iª$xÀé?kþµrÄ?iª$xÀæ?ïú{º~ˆ?eCñø?Fߟ£?eCñî?ïCEeÊ'?'™[{h¤?——S\†»d?'™[{h¤?ïÖbeÞÙ?qÞS,W?tÎÍû"F?qÞS,WŸ4FGL J0112.8-7506?ëûäûf!ÀDù}¿HÌÀ:ZíÍÎTŒÀ<'йÁWN@»Þû£yí?üž_ ÷Ç?ÅöX¡×«£?Ëë4Áӟz@@ìYZi@Þ+"ƒZ=¿Ñðh}—ÛS¿ä¡ŸAÏ-O¿à¯¤Ùš¿Ø5X§ay¿áá»;ªÐú¿ïè ÓI¾AGNbll3FGL J0112.9-75062MASS J01123146-7506179?ïjc ˜ó?a÷·ùé?'¼³›ìá™?a÷·ùé?ïºþÎf¾?Ÿ#y'¤W…?@LzfP&?Ÿ#y'¤W…?íÌRg±I?£(œ1ôÚ?±lÃòuµ?£(œ1ôÛ?`eß?…ֽűZ?¥f)ù¢3?…ֽűZ4FGL J0112.8+3208¿ê^,dVöÀ>ƒâCV—À83È23XóÀ;Äöƒ{á@Ü4d`§¶@<`Ÿ?u¾Ú,?±#™¸"pÃ@üm'ºZ@ÊwàŒGL¿Ö':ÛG¿áÿe:í;Ø¿åú#G,å¿å €sWæq¿êLÞÕãÌÄ¿åÄ|ÁNjAGNfsrq3FGL J0112.8+32074C +31.03?ïý3îa?/l50q?6`Œ÷oåo?/l50è?ïú-i£I?bK!V'«y?GJ[õrÛÖ?bK!V'«z?ïÆBÜÁï?€‡ŒŸòL?|ޑòŸj?€‡ŒŸòK?ïÿÎ*%¹Ì>ð×Ã~v"÷>øêí#åÍ>ð×Ã~v'H4FGL J0113.1-3553?ïþÝpËb5ÀTß«÷jÀ9Ûà$˜e½À<'4pJ@"{ZqÍ@¯ÎÄô'7?³îހº‹¾?¶ÞGH"íˆ@^á½Ùà@Sòt|(Å¿Ï<í[¸{¿àҟt¤í‹¿ãýDcÝ*¿é oA{P¿è?b`ÈAοïÿ4Þ®÷zAGNfsrq3FGL J0113.0-3554PMN J0113-3551?ïÿBH·Ëò?>²5¡ö:?¶éÇV?>²5¡õY?ïþZc—½y?H˜iiÜl?*YƄ(zJ?H˜iiÜv?ïÄÚÓÈÛI?¨c?}'–'\?¨f?ïÿ¥¨‡ûr>ÿf>¤î†?•Þ#5ý>ÿf>¤ìr4FGL J0113.4+4948?㓘oïIoÀ)ÒŸ˜·À8Ùì©&¥À;ºÇply¦@˜ãy·|@^·E|?¦Ñ›¯ô?±™é¾·5@
jÊA¤æ@èæ5?íԗœiW²¿ÜÎQÝr¸¿ã^ö€$}Ž¿ã}FA­¿ãÕ4ûE†¿çä]­Z@¾AGNfsrq3FGL J0113.4+4948S4 0110+49?ïý€+x?,–¢2TL^?3ü¤?Ù[?,–¢2TL˜?ïûÓèàv?c½e*Av?C"°\~'W?c½e*A{?ïȺ |Â?{ùá?~;¢ïÁŸŸ?{ùÜ?ïÿµá(Ï,>ôáX(±v²?‡µÌ4Û²>ôáX(±r›4FGL J0113.7+0225¿á¡îÀMûïÝëÙÀ:h†Úz4zÀ<rû@
faÞÂC@%iF·G?ÅbB¶3¿›y¥ÂÇ»?ÑÞ`þW@@}8ém¿æó0¿ŸÛ¿åNx¾­¥?¿çœÕÃìS{¿ãR&]·Á"¿äÜ¥‡äe¿ïÿù³>†AGNbllUGC 773?ïúR"k<‡?D`0ip0?Fµ²S
æK?D`0ipO?ïüoÇ'0?ZŸƒ«å?<Ç3n~K?ZŸƒ«Ú?ïÄwúýýS?~¢Bœ²å£?}āV#?~¢Bœ²å­?ïõ'Ôð@²?G;²a*ƒ?TúV~œã?G;²a*~4FGL J0114.0+6418?î¼®ü®5?ø£~éÐÀ:&xèI*À;Ëe±Ím@ ëW+5ý@)³(é-?ÅË#ÕGD¸?·£3÷(k?ìOQâJãS@=Šzº0?—p4£ý?ß&Á°¹ò¿âàKd'`˜¿×c§úÛR÷¿ç•¶ë¹÷޿׋²ü;AGNbcuGB6 J0113+6416?ïøVNÄs?PÃËáqÅ?N§žÄî+ö?PÃËáqÎ?ïðŒzú‹Ê?ˆX°ïÏW±?^ç

èmÀ?ˆX°ïÏW±?ït¹´Ê?'AZ¾«.þ?'hÉf¬Mç?'AZ¾«.ü?ïí[5R¨?U̘"BtK?b¤Ê­Wü?U̘"BtH4FGL J0114.8+1326?îr.¸B[–ÀH…S`Ð$pÀ9È=ñÓÀ<"HÏ|ª@%ôx7t6@ÔQ[<f¹?§JdR:	'?eŒQ1 áâ?¿ÝϾï"x@†ª(²ý¿ÜÀêm¬¿àùL`RP¿ão·]yØ´¿Ý×}_§/"¿ã:x øóò¿á5›WߺæAGNbll3FGL J0114.8+1326GB6 J0114+1325?ïþºÞ˜ì?=á¤RÐ?$Vòq>Ã?=á¤Rà?ïþ—]:U?CÊ	Xå?&Š.<Z®?CÊ	Xë?ïôvë…Ê¢?c'¯Üâ?x?W(ôj¼ñ?c'¯Üâ??ïÿh)lï?®öªš?RúÒaÝz?®ö©'4FGL J0114.9-3400¿á^¥ú9:€ÀT]§°³''À;_»QzÀ<¬zyBáý@!Á\+e‰?üÿéYËM?Á;–7¿ áŸlÂK?ßÚr\"Ô´@j¾—ÕÊ!¿Û2pžÎ¿èÕ?AßHz¿ß‰üÙ´¿â‡Ÿïôð¿Ëáw(Öc?|~Ó"Yú¦AGNbll1RXS J011501.3-340008?ïÿqÏ'…À?FqÅçO?ÆH%d?FqÅçO?ïþRvØÜ?H•Ãm<R?*؟rE/?H•Ãm<Z?ïøy­pÄ)?Y縛L'?NJ<ï\‹?Y縛L&é?ïþð5k¢¨?¤©]Šý? ü©EՄÄ?¤©]ŠÃ4FGL J0115.1+2622¿èwB}H#ÀB~|âÀ;Êön‡À<m|ßýa@8——¶Àq@MíHû?Ô3ÿ
z¿¬¨PÁŽ€6?åü·ÁLæã@
4rIs'r¿än?Ƕ¿²]¨@•5K¿é¿¥Ò.¿ÖKIàâi¿×*Â+A¿ðAGNbcu1RXS J011451.8+262337?ïþ:º˜p?-~½Û÷€…?,T^¶xòý?-~½Û÷€?ïþ3Ú¹z
?K€N­óô?,ÂTh_[?K€N­óé?ïÛÀÎãÖí?vi\Ʉ|?r˜Ž‰Ù?vi\Ʉ?ïþ¾v£Zõ?Å°Š§Ÿ?$•ÊP²m?Å°Š¨:4FGL J0115.1-0129¿Í¶:bæ~ÀOßbb˧3À:î¯÷ªÀ<7mƒ'˜@h€•'¢)@¶';‡?¾`¿øì?¹—´<25\?ò:e;Ãûm@6ƍ?îQB‰hI¿äµ€r'¿ë)ºy
2¿ìµÀÁ¦©¿ï'›??ï;-ÇüƒAGNfsrqPKS 0112-017?ïþÞ$՝À?$¢çûz…É?"²¦$~?$¢çûz…Ü?ïüæD¯o?]\•cæ?8Íß"ˆ?]\•cö?ïÒÀ-H
?s{¹	¯©Œ?vŸé[ùûõ?s{¹	¯©‡?ïû¢á'/î?5a^máë9?Aty»@K ?5a^máë,4FGL J0115.6+0356¿ê¹¶éáJÇÀM0—á2µ_À8ûá÷|þÀ;ø­•Ïà~@a$H¸@Go*ZG?¬
é½ôAÜ?²"†Òeh@X>»&²@\ìj!¿äa³'¿Ù®=•ŒÄŸ¿á1QFC±0¿à†&˜ðý¿æüÁâc¿á1´âf'AGNbll3FGL J0115.7+0356PMN J0115+0356?ï÷ÇXV»\?L3˶­)?PqOR‰I‰?L3˶­2?ïÛxYY˜ ?§áa3ê2?rCÓS3ð"?§áa3ê2?ï«Õ¾]›‹?‰敓d?…
h™4?‰敓b?ï}¨PiÀÔ?Íw$P?JõòÇå'?Íw$M4FGL J0115.8+2519¿à㳄QÀB›–À8¥´B'KÇÀ;¶Î¬ Ý[@Kn	È֞?þ¬*˅¤ð?£‹`-¸±?JïË
d?«*JX…@ãLÓi©¿Ô åΑ¿âyDÅ+áY—K
À¿ÛJÝÿz)¿Ù²†eà/¿Ý"o@ª•AGNbll3FGL J0115.8+2519RX J0115.7+2519?ïÿz"M?]NG$Ú?P¿M–^Ÿ?]NG%C?ïþ–RÐÃ?Asø€›?&šØó¿Ç?Asø€'?ïfâ?lùàÂi]?av\™~Ê?lùàÂiZ?ïÿü`8@Ñ>¹Û«Ì•E¾>¼þ=ùr(ó>¹Û«Ì•ï4FGL J0116.0-1136?ïÿ£NËÀR\/ƒ{J#À9Aª>-À<?¯à,ûâ@gÈ;B¡@©½R†?©!="±l?­[Žœ•Ÿ@¢Z2{@Êæºßr?›­5F¢•…¿â"Üöæ{Ê¿æ·hí)c§¿ãY`>.8ø¿æ¿Zž\!¿ïÿZªÕ+AGNfsrq3FGL J0116.0-1134PKS 0113-118?ïÿPI±?[Öx^Óë?öÞþ)Ԛ?[Öx^Ó$?ïýì–Ϥ"?J'¾G-?0›I'Þî}?J'¾G-³?ïމó¹À?wH¸ÓÜn?p»#z œ?wH¸ÓÜo?ïÿáÙúÉë>æ–VQ>î&6ËÐ>æ–Rò4FGL J0116.0-2745?àÊl?KíÀU ÃLŠÆÀ:ýayWÀ<Ÿ\>Å7­@!R'È>ô?ûšîcŠ	?͏t|©Ÿ?¾‰œKz§¼?ï
¾ßÏ3@" fQïýÁ̾Š?ïåt™/¿È"%Ú/5ù¿á½>!£¿¿Ø¥{úø.O¿ÔÁ*AÇöyAGNbll3FGL J0116.2-27441RXS J011555.6-274428?ïÿlñ&OX?¸Õxý˜D?aÛ6
W?¸Õxý˜9?ïþ;÷ut"?FÙo×å_¼?,@ˆ¨·¾?FÙo×å_Â?ïìuãº]—?mfß8Ö|B?cŠE¢h¡?mfß8Ö|G?ïûš;üQ?8¢œÄË$?A—ö¹ ?8¢œÄË4FGL J0116.2-6153¿êGyCctTÀK~r\=îxÀ:}ç&f¿À<š ]Øù+@ 3^(6Ö?üÈÈ@vÕ?»UÖ&"?´zڀƒaä?úcˆÕü÷?ýNá9–O¿ïó?']<?Ï\°¸¸Ä¿Î3BL«ª=¿áãyí+çå¿ÓQ‰_²¿âyUn"AGNbll3FGL J0116.3-6153SUMSS J011619-615343?ïós`
w?[Z
€ØL—?Y?Éëy?[Z
€ØL•?ïôg¥#‰Æ?iÎÇGݒ?W0µ¸ìw†?iÎÇGݖ?ïÃ&1Þ̙?€7wnRɜ?~l癳'?€7wnRɝ?ï•-؅`?z¸$I-Š?Š¹ô‰Þ¨?z¸$I-‡4FGL J0116.5-2812?ä"¬¢?ÀUÎÙ‡+À;Zm]ÑloÀ<šVHáñ!@õ^*Ü#@ƒlØ?Æwe'+O¿¯]ÃT¨ù´?ãüµþT.U@ÆÞþ}Ÿ?åɛ?-±¿çbz¿å"u'ÊIe¿äê•ÀF+³¿Üãa¹®b¿á~ÁqN÷µAGNbll1RXS J011637.7-281146?ïû9Ùž?::V~:‹f?A¿˜é}?::V~:‹s?ïüùQ!Bq?Q
Bç	£&?85võìn7?Q
Bç	£*?ïç‰^´lš?të,âm £?hv¡K"eˆ?të,âm ¤?ïü|t~º`?0o®­žó?<\
-Õ?0o®­žÑ4FGL J0116.5-3046¿ï˜33ö/ÀTÙp÷¹àaÀ:üd^NiðÀ<¦ù)L)¤@»Ç{)@˜jßqë?Íåw©ïÏ?ÃD͏jk¯?ò\T)Md@ˆ|ñm@?ívѧR¿ã"Q´þ¿æ¾ç0ü!N¿ïþŸ½Êü=¿íjUéŸì?ì0…ÔÀ·AGNfsrqPKS 0113-310?ïý>Œã¡?:KðÜŸÚ ?7Ö˜âûÐ?:KðÜŸÚ ?ï¹/‰å?'Àn•є?¹ô†¿Ô?'Àn•є?ï:ÿ«Í?Ä?¼5»Y:3?˜ 
†X…?¼5»Y:7?ïʐê	Å/?o&¯:3£?z·Šûhõ?o&¯:3§4FGL J0117.5-2442¿í\Ïc×ÿzÀT颣Y6À;ÁV¶JªÀ<ïCœ7Ì@!W"È×Ê­?ñøDIÛì?é!—c•?ބwžr{?ñ+k…L?ý;IÚ¿~±¿'¢Ïù'Ñ¿éôöí1Ç"¿ïí	þ±vZ?Ñh=¿çTbøóœD¿Öà¤E9¸AGNbll1RXS J011746.6-244329?ïõ}ðDd?XÅW=D;?UÉw67?XÅW=DH?ïûD$+±È?`¡tÜÓ@^?BïoQ8ã˜?`¡tÜÓ@^?ïyÖ^'Œ5?(qh'Ÿ?Å4/®yr?(qh'¤?ïû|2Ï?G¨ŠáÏâ*?Cö4ñ¿ê?G¨ŠáÏâ.4FGL J0117.8-2109?ïÞUòázÀTa¯ž¾œˆÀ9lszKÀ;æK!JÓ@ÛBV¼¥7@¨¾e*ý?¶ú³åË z?½j°£vg@ý¾`l@½X~qJ?ïú"Àā¿×ÅÑZûú¿ås^ ò"Ü¿å锹`~¿æåªda¿ïú)âQ™PAGNfsrq3FGL J0117.8-2113PKS 0115-214?ïþnóÍm?$¿ž<bËî?)Ã)?$¿ž<bÌZ?ïýTšWª?T›k3_L?7u[-B¥¼?T›k3_L?ï}¡««þ?†uâO€í?K݊Š€;?†uâO€ð?ïü66'¥~?1é7k2p?>NKrÔ(?1é7k2®4FGL J0118.7-0848?ä¿BHrÝÀQ¤Åm\ú­À:nÀ<~lê&3@MùÛùz@ÐÛä—Å?Ï1æÂlK®?Ò\'þw•@ùCM\ª@	Q¬«5x¿©È&ÊÅ
·¿æô¼U…ÿåë澚¨¿íb(E¿ïÿÙi"A'¿ã.<=óÖ|AGNbcuAT20G J011844-085058?ïþf!x"?(¨å8þÏ?)ïvÅ|?(¨å8þq?ïßÈÊk¶¼?"Ž#ÒòÔ?pšÊ$¢©?"Ž#ÒòÒ?ïP+úè4?ŠšË‡,³?•ú€¢íùƒ?ŠšË‡,®?ïÅý‰8À˜?l¬ìG´b?};cŸ´??l¬ìG´a4FGL J0118.9-2141¿ê›_5ÀTnð¹À89¼R+EÿÀ;ƒ|@Ã@æ-Lê@œIwB?‡B÷Bä?·dD"@;p@Ú»£@P;\Í`q¿Äy
t­¿â<i"‰G¿äÄFwÜ¿â¡fµN+¿è6;ÏÆ|¿èéQ'©"AGNfsrq3FGL J0118.8-2142PKS 0116-219?ïì5´0ÁO?c¯Iñƒ$?cÊKÏ>±ó?c¯Iñƒ)?ï¾È#­"?©¾Š._r?€M÷ºÛ†?©¾Š._s?ï†Õß&[å?Œ€Çjëñ!?ŽJˆ6i?Œ€Çjëñ"?ï¢ÞÑ}'?|ËVª¯®?‡H\ ¶&?|ËVª¯­4FGL J0119.0-1458?Ç'(ŽOIÀS†YJôñÀ:I£–ržÀ<V>Eµì¶@ {ßaúÆÛ?úgJ&"¿??Úl'p‡R?¾ÀRëà8d?þ1Ó·¢™@ÛEPl)?ï÷Ÿnc‹¿å2GzèÔj¿Ý¾6|=é¿Ñߢ'fŸ¿Û¬ß\‰É¿âÊÕFEAGNbll3FGL J0118.9-14571RXS J011905.4-145906?ïûb{§˜"?Q
ubwq?Bvaª:?Q
ubw`?ïý'ðFÛO?QdZðùG?3è}É%ŒO?QdZðùGŒ?ïçÝJß?tÒr|¥D?h"áµ ê.?tÒr|¥:?ïç¶Ñ>n?U?<|*?hI.Á'÷±?U?<|24FGL J0119.4-5354?ŽM¸±ÀÛÀO[ñ•1äÀ:ÙܲÀ<µm¿öûu@×o'yÇ@Â/BêÊ?À‡‰v¶Àœ¿¨§q@˜y?è[x¦@Y
\J?ÄB§Yö–u¿éqmŒ¿äüÅd"¿¿ßD˜¶DË¿ïóO]`XZ?âM‡rO¨µAGNbcuPKS 0117-542?ï쀿¸¿<?dÚEî'	?c@G@Ä:?dÚEî'?ïìjœñ/©?x›â?c•cÐW¼?x›â?ï½|>KRª?~Kº^M²?€ ðm+UÆ?~Kº^M²?ïèïŸŒB?Z˜ü"Ä?gb`s¿N?Z˜ü"Ä4FGL J0119.6+4158¿îÑNµzÕÀ4"ó#x«
À;DÛ;$™<À<¥ˆI=‹@¾½º`8¥@Ÿ°ºG?Ð'L†@?È¿ˆ–'ýC?û®oÜV?þC,»–ï?ï= "Ds¿¯´Ê!¡»Q¿é6†…ÀŸ¿Ü»õy"@"¿í5Á¸œ" ¿ïÿX¥³ƒPAGNbll2MASX J01200274+4200139?ï$Ì$
^?›i¸'O>—?›f{~½"]?›i¸'O>—?îhnPŒ¸?¶ázW_¶?©é÷4p?¶ázW_¶?íLn ÞÖÃ?¢
ð><b…?µœŽù	Iõ?¢
ð><b'?ë®&Ѿ¬°?¦)ooHÞ?ÁGd¹MD?¦)ooHÞ4FGL J0119.9+4053¿ïëá6hÀ5¨¡œZÀ;œqÀ6¼UÀ<ØÐÜüŹ@ ÄLˊ­?þº"Àõ(6?Ø:ú݁O÷?мXáB¥—?ú*…ʯ¼@`ô)2(q?íÜã›EkD¿±uWELå¿Ûç};?¿Òuác\ƪ¿åÙþí[c¿ïô ~$É
AGNbcuCRATES J012018+405314?ïéöõ"G?c4ÀqÆn?f	
l÷¸O?c4ÀqÆm?ïð?®fç?†Žçÿt?_ô£234?†Žçÿt?ïj1'{Ëú?îm(€|?'¹Í°†€¸?îm(€‰?ï^À{o§?Ôû,n?"'ð'1?Ôû,m4FGL J0120.4-2701?ïý(Iæ1ÀT⹩çÀ8dµ—&À;YАä¿@øŠë«à?ý#8ê,Y?âWùf2å?ª²³_ؤ@ñ¡˜kœ@§é2Þúw?ïýŽ5¸H±¿ÙCSy¿Þ@áDž»¿ÚtZe&Jm¿âXQ€%TM¿Ü˜‹<3·èAGNbll3FGL J0120.4-2700PKS 0118-272?ïþl‰éR[?.† ñ+v™?)7ajÚ_R?.† ñ+vu?ï್¥‰?šì"?x§¦9-;"?šì"?ï¢#ׯ¦.?Š"p"æo?‡w
t"?Š"p"æm?ï'@"UÂæ?zyC|õÏ?‹oÛ*F•?zyC|õÏ4FGL J0121.7+5153¿ÛÈEӀ¸ÔÀ%dí0µªÀ;'³ S\žÀ<ˆ §ªÔU@"€±ˆx´ó?úï'åJr?ˆZ!´†?À"ÈVñSj?÷V%¾@Ø!ÈýŠZ¿ïÿÀ	oëJ¿ïuÞ©n#?ïÿXJ¿¼sîdL/Ù¿ç
çIOÕ*?"™N›Ÿ´AGNbcu3FGL J0121.7+51542MASS J01213367+5155520?ïþÐtµª?a´Îz@|?"ø¾¥NB?a´Îz@?ïùg
Í7j?lȖnMÉ?JcÈË"ZÝ?lȖnMÉ?ïéyí²Å+?jó^(??f†M:Ô½?jó^(-?ïµk>Ùn?zïKµõÃ
?'¥;0I¤Ñ?zïKµõÃ4FGL J0121.8-3916?æ
"²+4ÀSyB=KÀ:¤ù8e¢À<›"´W‹@ "]8??ý"6÷
7?À—ða§dÞ?µ†
`:Ó;?öàÄn&N@qÝn°ŒÐ¿Öp¨ÿ¾Ç¿¥†K3/,¿Û¶\þˆ±•¿Ù›¨B›†¿æ'ø»h {?qs™;*AGNbll3FGL J0121.8-3917NVSS J012152-391547?ïý17º{?0PÀ¾æÝ?6vB,#{m?0PÀ¾ç
?ïüX-Éȹ?W™r€n~?=>'±º2y?W™r€nw?ïñ˜Ò‡Åý?g2ËñÀ˜?\ÎZðt	\?g2ËñÀ˜?ïí—‰\&?S¥	žëÍ?bçhv£Ù¯?S¥	žëÏ4FGL J0122.1-3004?í¿ÀT©Ù¾L×IÀ;ä¨+,ÔÀ<ì·/¡®@#%oÑ@?÷jðSº'8@m}aT®®?«ßXVÍ?þú¢ Í¿¿ÎŒm?îÀÎۚƿéX•";"+¿áW7T*#À?™Á]=¯?ÄÙRíÞ5AGNbcu1RXS J012203.6-300507?ïýÇÁkž?4iíœý*¬?1Ç	ô£à?4iíœý*Ê?ï·FòÀ±Æ?©¶…wÏÍ?'.COӎt?©¶…wÏÍ?îô{M-]?¡_¸eO{? ¸K-.?¡_¸eO|?ïóÿfkx_?füSç¥Ø?X3)E)?füSç¥Ø4FGL J0123.1+3421¿›ê€Î7ٗÀ<†Â&€À:"Ž;—…ÃÀ<hÉÒ*Û@!¢Ÿ.ÙÝ,?ú~V²"<c?Àì²nì?œHÿ´øè?ßøüLl?@"dQ›©¿ìb>ƒÉM¼?ÐÛZV¢¿é̒ë)¯&¿™
?þÑ4¿ÒS^a_@'¿Ðg\…'ûAGNbll3FGL J0122.8+34231ES 0120+340?ïþLÞ8TÕ?*Á'ÙÇ5n?+2z²ÅH?*Á'ÙÇ5N?ïþè{*¥K?>%àZ©+ú?!xMU«`??>%àZ©+ì?ïޏdeÒ?z ¾ŸŸ6?p¸MÍøe?z ¾ŸŸ4?ïüñ¨°¾?+õ	ßU?8rºzÇ|?+õ	ßB4FGL J0123.7-2311¿ßJ3çf†ÀTlÎþÖ4UÀ9ÊR:_w_À<-S±Wü@@ àÚu×È?ýmºßd?²'ØŸ¾Ì¯?˜™ظÏ{?è¹Nª@ø/Ó¯¿ð?ð¿Ü]aÚæk¿ÝI|`Mȋ¿àB¦¾EJ¿Ê¡½?6.AGNbll3FGL J0123.7-23121RXS J012338.2-231100?ïþ³›?pÅÓ†?$Î/O^?pÅÓ†`?ïüb‹Ûqu?[ÄK"©0?<ë¡$t[l?[ÄK"©0?ïèî¹éÞý?o¡ùv·æÕ?gF!ä?o¡ùv·æÒ?ïõ÷7,"µ?IÉ4ï¼?T'¦ö—:?IÉ4ï²4FGL J0124.8-0625?ã62C«ÎÀPõ7óŒT7À:"t•À<Œ›'8S@[ÅßȨ@'tý¾?Á¾«·ShÞ?¯Z"|ýŠ8?çi%}½ðç@ž•Ök‡
¿è[#aÙ丿䙅½nµë¿ãeØ!Ëå¿â²tý¾¿à}¯XGÀ¿ìÏñ¿öO¨AGNbll3FGL J0125.2-0627PMN J0124-0624?ïÿ	ŠpÃ?1iƒy*¹?Íî±ç›?1iƒy*²?ïþµÛ=Ÿ$?CЭNöSP?$¢L&
Ƭ?CЭNöSY?ïòÝQϯ?i4EÛ;s?ZEù\`¡Ø?i4EÛ;s?ïÿ›ã:—`>ÿ&Ø6ۂ?	1Z'âŽ>ÿ&Ø6ۀ¼4FGL J0125.3-2548¿æÄ{"=ØÀT'†@ €À9Û7ƒ$OÀ<wÎaøBœ@NX"¿åß@&¸0]•Ý?¶Økš,?µfmrIHž?ýS
3_¨Ý@	Ò<m™‹'?ïšáBO°Â¿áŠ6ðW'¿à¢ªßè'¿âìeïH"¿é.xMïw¿ïþ¾P¤]AGNbll3FGL J0125.4-2548PKS 0122-260?ïöTÁì:ä?aMË~-2\?SV|'Š7J?aMË~-2[?ïøðh"•?{7ž´€K?O´>]í¬;?{7ž´€L?ï´ÞRcè?›I<r?'Èk_§&?›I<p?ïá75N'?`aU1£ &?nèÈʱno?`aU1£ +4FGL J0125.4+3200?éB{‹(ôßÀ>O…r›(À:o€Ãþ¬À<\\3Ý}@륹¸rù@­"BJ'k?ö9¿‹P?ˆ?ºPVڂB@ÒL(!²,?ï½ö=	¿êÊáÛQÊοìNß+t"¿Ú%|ª¤¿é<¢¨6¿ïøHEéïAGNbcuMG3 J012541+3152?ïþ¾ÝÌÂ?$BqÅ÷»?$#3ÛC?$BqÅ÷»?ïúµëÖ?a^Iͦ?Gï…(P«ß?a^IÍ«?ïÉø½èý?€ˆC3?{¡v‹w?€ˆC:?ïù‰ºÐsÂ?@»ÞFv‹*?IÙ¾0ú?@»ÞFv‹4FGL J0125.7-0015¿ïÿú‹Øg6ÀNó¼ÓZ…ˆÀ:>¨*VàÀ<eŒÿWc"@ôÀÙú\Ó@T‹<߄_?ÀÆÀCQŽh?µOm¦v¡È?îʾ­	c?ü©NM?ùÀ¿ÎÈ^éooÏ¿êY9W:¿éµO!ü)1¿ìn•	 º¿ïþôœõn­¿ïÊO[–AGNfsrqPKS 0122-005?ïû§ûpê?KSÓ5!|?Ac€<[T?KSÓ5!i?îøÎñf±?¯×n¯ò? sé"ï?¯×n¯ò?ï–ä£äY?•*LÁv?Ÿ#kƒt¬?•*LÁv?í÷	U5?¡@éN>¼>?°GµSW¸?¡@éN>¼?4FGL J0126.0-2221?É&_;‹]ZÀT3 ù	kºÀ9ú¤û¨'À<^–ªÑÐB@
'èý/@Qè´k­?¸çý)áÐÀ?¼Íé'e"@Tá@ùòìòB?ïdcâ}Ž ¿åÄ ]Øù+¿æ58%á;¿ìŸõÔ-¿á:ҙ•gÜ¿ïý› Ø<ÂAGNfsrq3FGL J0126.1-2227PKS 0123-226?ïÿ_PÛ?yy	L?|Uä–,?yy	?ïþ
µõ?JÒÖqÕ?/.®t ¯@?JÒÖqÏ?ï×&!èÔ?r|³ q?t}ìï–?r|³ w?ïÿdC ;?}חY^?3w›ø?}חY]¶4FGL J0126.5-1553¿ì³ÆÌv"ÙÀSæ¯ÌâÀ;-Ù8ëÙØÀ<™Zž²O@9`<*Ô?ÿþøþƒÿ?ß±‰ÚÀ?ã=:ZMS?þ'PÀô*?þÝAאË¿ï•'¾´V?ã"; g~"¿å"]9–û¿é(ª^û'¿ïý}Ú rf¿ÑÓTÛúg:AGNbcuWISEA J012708.49-155554.1?ïh/Ow?•Á¡2º"×?'ÿºQ'?•Á¡2º"Ö?ïˆÂ$´ùR? ±{
EAx?ÏvÒÁ«`? ±{
EAw?츇+Ñ¡?£cY$šf?º;Ç¡rù?£cY$šh?î/ßÙU_·?¡AZÚ¥ð?­jª'?¡AZÚ¥ð4FGL J0127.1+3310?ì~§T0
À=~À¨À;MPïܹÀ<±­ÂEŠN@ wzÜÀ	ñ?ÿ:ŠÅÁ?Ñ?Ë)¬ ÚÁ?šúv~6'·?Ó°È_TÏ:?þù$f'¯j¿î̞ßS¸?ï—L¸?w¿ãþÊuÚx¿äWewS´¿Á¢@Ýîz¿âÛea-Â[AGNbllNVSS J012656+330727?ïýL»öj?3Ù!Ä)7>?5š OÄ´Ë?3Ù!Ä)7X?ïü)³¸
)?a
9uû5?>²b?®µ€?a
9uû.?ïݑkÖYH?rIUÊ
âq?q7JÓ\p?rIUÊ
âf?ïî:¼žÅl?VE{YÏç?aÅCa:'¼?VE{YÏÛ4FGL J0127.2-0819¿×¸œ®N†ÕÀQXh‡¨ÖMÀ9…(šRýÀ<>EJŒì@°áõ(
¶@ÒD}ÞR0?²¦¶¸ŽQg?¹	ÜÞÎé@ìÜ¢,æ@¦+
DÒm?ïÿá—_,¶¿à2f9Œê¿â?™s,Û¿ã­_I;³¿äÀÉë£R¿ïüäÝdʅAGNbll3FGL J0127.1-0818PMN J0127-0821?ïߛ:]"?o½~éTH?p2bòQ6G?o½~éTA?í³Æ{é¸ú?Ã<iÉ+–º?²aÌ ²8%?Ã<iÉ+–¹?í®¶/2"v?¢É,r<]c?²ŠN†kÜN?¢É,r<]a?ìs+}ŽdÏ?£¼ïã;?¼f¤ŒÙ?£¼ïã;4FGL J0127.2+0324¿ÔŽ=5ÔN§ÀM ÖÓõ¶À9ëRV)ŽÀ<A¬½ã%@ª—mÅU?þƒ=¢!þX?¸–_×Öì?©"U´?òŸ£ž\w@XS­&>X¿å¶À'¢Ü¿ÁfA''–¿á,Xï
¿Ø͙ÞA¿Þ"â¨V¿âôN>aAGNbll3FGL J0127.2+0325NVSS J012713+032259?ïÿB®r=?t…xn?ª1¸\ž÷?t…xm?ïþvFe[a?D–YQ@=?(›™ªIéÌ?D–YQ@9?ïöùë}K?_DŒí-‡?Rx©ke?_DŒí-p?ïÿº?´Ä¿>ôâO"Óþ9?pÎÐã>ôâO"ÓûG4FGL J0127.4-4813¿à:ò†€"ÀPñ(Œç°À:¡îàªÀ<±HÒé4@6\>šD@¬u>p~?½¬Žé½Hu¿›íµ^\µ?ÝxÞ8/v@[–ˆB.?Š&Ã‰à¿ééŸ"w¿å¶?A´U¿á¤•á~4¹¿ïÿü¥¬¨?ïÿÍ
	n>AGNbcuPMN J0127-4813?ïþ?z	gÃ?(?Q{V¥–?,_iƒêô?(?Q{V¥÷?ïüÔ^ˆ?c-†Ã.T??Á]¿ê%?c-†Ã.T?ïä=
·Ü?r·_0à?kÂòùH#Ô?r·_0ä?ïüfÀ$/ƒ?1"·Ñ28?<Éþރí"?1"·Ñ294FGL J0127.9+4857¿î×µþbU«À*÷´ÜëÿÀ:9ƒ^ıuÀ<%'¡}"@ãþàEP@؝jßqë?½"¿Àéz¿*ò¿Gœ?Û÷ƒÈL
@v¢ÔUØ$¿Å/"Â͚}¿å"wvY"±¿ãNU}àÖo¿ê\ \–ÙÌ¿ëEMýcîg?ÖºqëÕ¦AGNbll3FGL J0127.6+4851GB6 J0128+4901?ïûIŠ=Ã?D‰ªrçÏY?BÙ×óê…?D‰ªrçÏc?ïþ¡âk?Fz*¿Ç?%áޙH×?Fz*¿Â?ï¤yö"?ˆˆú¸1S?†á'_žÿ™?ˆˆú¸1N?ï÷Ž5?ò?@Y˼¼Â?P㕁7?@Y˼¼Á÷4FGL J0128.2+4400¿Ý/®|À2^ê šª;À:ñJ¤iuÀ<gÕÈc@}"‹›)@2mæÎ?ÒÓJàxü?Þv­*@pZ:Þù@'N¤RÛ?ïùHUÚ'(¿â£«€ÌÄ¿é	¬AU¿å
" ®¡>¿ïÿ÷fÔJp?ï¢O¥YÁAGNbcuMG4 J012818+4405?ïä}¬(V?u«p"À
?k'SoשÆ?u«p"À?íÞÄb?¼{/ÅQj?±	ßï/9?¼{/ÅQj?ìž/kã‹*?¦MI·£?»" ã¦²?¦MI·£?í0Ý­D°Œ?¦D'oë‰æ?¶y•Ú{œ?¦D'oë‰å4FGL J0128.3+5710¿äºôœ¢ÒkÀ^ÒàD²À:…	ËZÝÀ;ö÷ÛnP@@Ê?SÒæ@f–DzƒT?ÀË0šÁ¸¿¨tæ†Ý)f?æÊÐê°
@6hk#d‰?ä?}ïD¿á©ýýÇA¿éÖ.u^Q¿çÀÔÁÔi¿ÄÚWåD<ñ¿äMHˆ/AGNbcu2MASS J01282987+5712494?ïùGÁýä?CÍæÖYÄ?JáÀøl9?CÍæÖYÜ?ïþ»V½Ú·?K¦&£?$J""TœÆ?K¦&£+?ïË·d4df?z#ËñWëÐ?z$MåÍ͂?z#ËñWëË?ïø-§æÉD?A,[¬ú:?OI`dÚòå?A,[¬ú"4FGL J0128.5+4440¿à&nhÂÆÀ1±Û˜AªÅÀ;"|úÀ<ŸÍHÏD@'³Jß@£a™x?τ"ú£tº?ÒÁqºWC@÷~0‡‡@
^~\&q"¿ïÿ	ËZÜÅ?ïþ¹ä'¼0¿à~ø=¾Òc¿àéÔå i¿âËNÀŸm¿ïýjŽê/AGNfsrq3FGL J0128.5+4430GB6 J0128+4439?ïýóJ'ù¨?+XA‰Ñ?0e«è2¹Î?+XA‰ÑE?ïöY;‰ò?sOS‡Ecú?SMˆìÆÏ?sOS‡Ecû?ï]ÝC›Ëå?ŒuÕÊÎöC?"DWŒ†ƒ?ŒuÕÊÎöF?ïՙW°(?e?}Vô¹\?u3~Ô'ì?e?}Vô¹]4FGL J0129.0+6312?³_Ž?äÇ|Ìy1À9VÚÎO¨À;(Âñ·ü@)Ûp©‹@‰‰>ÃO?ŸIO@?ÑÏᗊ @"ßBñX?þ[^¸ù?ê|Iâ¢!(¿ÜJÐÞªDã¿è+b€=¿èr(;ˆl¿ïþSÝͦ?B§D}AGNbcu3FGL J0128.4+62572MASS J01283059+6306298?¶TmWŠ'—?·dNQ!Ÿ?í5rU»?·dNQ! ?Õ¸ËX"•?Ö+ácF•:?å#šSúnµ?Ö+ácF•:?Í#®ˆ?³…{u¢?è·?zT^?³…{u¢?ÀœÐ°€?¬ÁUÏüú?ëØËÓßÿ?¬ÁUÏüû4FGL J0129.7+3436?ïÈ}"UÀ;—{Zê1bÀ:ΪcyÀ<¢|(oŠÒ@©…©	¤?üYo!öÊÍ?Ì2T¦uu"?ÑèßZ©š@ÂE¿ý±q?ü;ÓÐÍŽ¿í^¨âŒÒŒ?ïÿŠ#ÚМ¿à?(¿'ÐͿێÅ?º«¿ã;½pcj¿ïþ2Ö!ªAGNbcuTXS 0126+343?ïøA³ÁéÔ?TçÔÝ¿–?Nù0øX·™?TçÔÝ¿–?îh~öÍ;Å?·föâ01?©x",C«?·föâ01?îx?ÓuØ;?›À	ÖM?¨|È¢|O?›À	ÖJ?ëïríë?®ïÅd¦~?ÃÌB4HSœ?®ïÅd¦~4FGL J0129.8+1440?…•ªË">ÀG"ÇŽŸj"À9ü¹w…r›À<UÍ&Žà@‹]†6@ø6Ã
¬+?¼÷¾=?Ňz]>J@8âe+Ô@uÏm À?áÛނ׶5¿äÄÏ"¢À¿ëSÕ£Ï(¿æü":µ´¿ïÿØ'sâP?ïýgr0õAGNfsrq3FGL J0130.8+14414C +14.06?ïãaB™Ô?q¬a>¬€?lžá½f+E?q¬a>¬€?ᄂ"?–,éÔîiÇ?€yÖܛ]?–,éÔîiÇ?ï0
s?•1ôkðê?žmùþQe?•1ôkðè?ï'hÌ5ú©?÷ܲƨÔ?‹¥ÌòUV?÷ܲƨÖ4FGL J0130.4-2129?ì7áe·ÀSޞ²gÇÀ;8Ov_ÙÀ<Äå°Éa@ 90ƒUŠv?þK¡ô±î$?Ê,ëš?®.‹qYM?à…{ÕctD@xUy"%i¿ïø•½ìà?ïÿèþ†®/¿æ/:€.¿Ó+u¤œ×è¿àqÏP4˺¿â•=×AGNbcu2MASS J01302573-2128389?ïÿEßtló?Ç\lvk|?Dra‰w?Ç\lvk7?ïù¼ây~?fÏ5
è³?Iôv>?fÏ5
è³?ïðƒÝÜ¿?cQÞB³ßz?^øDFã?cQÞB³ß‡?ïõbf¬±?Kµšk	ü?UÉ;2¦Ÿõ?Kµšk
4FGL J0130.6+1844¿êJõ¶ðÓ ÀE"C•%À:·t×Bq•À<zd׍@D§ú°`@؞wNëö?½£‰¤^¦Š<¿f?çm°r#3?ûÒÖ+›9W?ëÙßYí1¿ã¼§ñK1W¿èy6ýîü¿Ùö?¿æËxÚq3¿äã߸âµAGNbcuMG1 J013030+1843?ïí®ÂÅ<?V/n§H?bQñ=:Ã*?V/n§C?ïÏ'2''Å?»(æÃZ??xlf¶ìŒ?»(æÃZ@?ïÈ3:UÝ?y´ç‰MOK?{æsâÕ×?y´ç‰MOD?ï|ºÚz%—?wv»K—i?h¤°»MK?wv»K—h4FGL J0131.1+6120¿ÛƒŽ¦	ó¿ò¯bXº¬9À8Ê&LšãFÀ;™Ô	×ð@ œxfn?ú'ƁY0ô?«_§/"R
?´dsá½äk@mgŸKŠB@5êhi ¿ïìk˜ÕN|?ï5O؅g³¿ÒÑ@"ªt2¿Õ¼`Ï"½¿Ú\"»;*¿×fq#-×AGNbll3FGL J0131.2+6120RX J0131.0+6120?ïþõ®¥?ðÑ>ñ? ®õ©Û?ðÑ>~?ïBåžÈ¡?µ¥PÄÆ?—£L&ëÝÊ?µ¥PÄÆ?K5hV?ýo)'Ý?Ú-2¥êd?ýo)'Þ?ïëæâñ{?VkéÅLsÞ?d<N"¿?VkéÅLsÝ4FGL J0131.2+5547¿îúÓν£À›œÆtÄÀ9Ѳ–À¡EÀ<Úìô‹@	²:zOQ@Ç>'Ä?¶)G!&Á5?' Cò7?ÚÉmÝ(9°?ðìÌKós€?ëÓåjR"¿ÒD¬{*C¿ä"éœl_¿á¢>ƒÉM¼¿áèi«•D ¿á?áíEhAGNbcu3FGL J0131.3+5548TXS 0128+554?ïɈýù'û?|«;[îù ?{;7a?|«;[îù ?îÀ‡¶ƒ?´O	RF7,?£÷"—ήŸ?´O	RF7,?ï€}¿µÖ?‡dý'ù€?àŠ}p?‡dý'ù?è•Î™>?±Œ¢kxÕ[?ͨǡ›Æ?±Œ¢kxÕ[4FGL J0132.7-1654?™`ðØBüÀS0#̎À8qŽ©{ŽíÀ;âêJŒM@»ãr€¦@&ÝA‰?œS蛛¡?¯" î@UL}‡\@:T‡–·½?¨­[ î*H¿âgwÞ]îÉ¿å"Â<Pg¿åfÿš6¿æ-À×K+¿ïÿƒ}ùUAGNfsrq3FGL J0132.6-1655PKS 0130-17?ïþ¨˜ƒ? ¶<22ÿ?%v§Î"ã? ¶<23:?ïü·Z,Os?Q&.˜Wü?:E."pò?Q&.˜W÷?ïÎêð»1?{«¨ÃÙã•?xŠ÷‡¢h?{«¨ÃÙã ?ïþ±­Üž?ie
w?$å'â6*5?ie
\4FGL J0132.7-0804?ÖÆà_³ÀQ%EŒÒ
úÀ:½%eëdÀ<{Y"M@ >_W(…Û?ü4sT‹r?ÆlN'^?ÂÌP{£`?ý9ƒ)Ì@?ûdÚ­‹¿ïÿù&Çë?ïüe@Ìxê¿«{ŒDg}¿ß,ÐÃ|l¿âªo¥Ó¿ßæ‹d͊AGNbcu3FGL J0132.5-0802PKS 0130-083?ïõ§y?THX*¬6Ó?T±
ßÅÜH?THX*¬6É?ïÔW 'Žó?‡ôÑFX`?uÔ/·8†¨?‡ôÑFX_?ï˛²ƒÉ?y->æEî?z2&ý>|?y->æEì?î܁Õþ'?'i¹Dü<%?¢7â ß©?'i¹Dü<&4FGL J0132.8-4413¿ïòÇ&¥íÀQ¿!>>)0À:W]$žDúÀ<¬wD@œÒá¹ÃÜ@"¡ã6ï?³"jŽSš¿«¾Ùo˜g?÷ûƒ™}?üSÙÆÛF¿ÕéC¥ò¿ç5ø¿ßHƒ|vÉ
¿ãÒ. ý;*¿è›_Óû?Ðؗ;ˆBAGNbll3FGL J0133.0-4413SUMSS J013306-441422?
'ÿ?Š·I~羊?ŒÝÿý[@+?Š·I~羈?ï²Ï»?"ñyFŒ?ƒL;X¿œ?"ñyFŒ?ï"E*99?"áGq	Ö?›·\ú¸Øæ?"áGq	Õ?ïjä…œ?'§[€ÂƬ?'£o\Œ|¯?'§[€ÂƬ4FGL J0132.8+4324?ÞnqÙlçÀ2ÔUGZ2À:œ½‡µk‡À<~ÝW^‹§@Ÿ™¯i·@|¦ˆÃ?Å覺YX?ÏèªäD¸—@*%£'·Õ@Q»úA¥¿êN›n…ð?×ò)é•ö¿æÜ¢˜E܃¿è6'@Œ¿ç¯§"X¼¿Ò6ÓfD¸AGNbcu3FGL J0133.3+4324B3 0129+431?ÊÑH?­µjm84×?§'ãRë~¸?­µjm84Ø?ï¿SÚ
u?˜ï7*k)?€+	||¢°?˜ï7*k)?ìÑeðG-"?§øll-BL?¹tÐ}ƓÑ?§øll-BO?ï{*$?†!d7<&9?œpš»}¼Z?†!d7<&84FGL J0133.1-5201?æôþ>@:ÍÀOó'½RÀ8¸_b"À<Ûä—Ä­@a–8¼@ÐlÚ"?¡¹nÝ>›,?´ØœŽÁy]@}<y-ˆ@zdËÍ¿¸tsß²¿á%ĵ§Z¿åŒÙ݁zê¿äIê.Ýc¿ç-""aSØ¿ïÿGþò8íAGNfsrq3FGL J0133.2-5159PKS 0131-522?ïÿ'"?>--Ë?¿}ÍÍsQ?>--S?ïüOsS·?V2i.€ë?="ebGlö?V2i.€ë‡?ïÙŽVŠÁ?xo6špÍ:?sp8Ôº ?xo6špÍA?ïÿöE>)ú>Ï%‡5'U¬>Óuƒ¬
ݬ>Ï%‡5'LÓ4FGL J0133.2-4533?˖Bîڃ`ÀQrŸ˜·À;·.Hè§À<ÿ'zç&ë@!Í\áb0?ìišÎM?å‹ÿ'=?åÓ°ìœuí?þëªX-¾?ò'.䬿ÙäŨ¹?í,{ž†é>¿í¤.}ÁÌ¿?ÒÄîý#VÇ¿Ö+ò¢xf¿Õ>ºÛˆ§YAGNbcu1RXS J013308.8-453528?ï{‡³²¶)?•à	֌÷?	‰©:Ó?•à	֌÷?ï˜';¡?²r·†oJ?üϸ‹æ?²r·†oJ?ï_µã³k?"0Ù®|Œ?ô	C‰'µ?"0Ù®|‹?ïEÞÕî?'W"®>Ð?—D'B<j?'W"®>Ð4FGL J0134.3-3842¿å˜PDŠÕgÀR֜wškQÀ:í—û3èeÀ<ÆÝåùÄ}@åçØkç@n£f¡õ‰?ÅEp!¦?ºd]þ7ÿ?ñ oÇ88V@-âÃJb¿ÎY	†'¿ÖZ–d
0¿çD[C¢¿å[«!Z¿ïý¶¿oA+¿ïþë-
$FAGNfsrq3FGL J0134.3-3842PMN J0134-3843?ïþò&/?![¾Ñ\? ݞ.]@?![¾ѐ?ïý u€$R?Qzc•'Øg?2üSþÝr]?Qzc•'Øk?ïÆ}Ø)?xü	¹£À?|Áýk9?xü	¹£À?ïû²r?5ȏ½ãá?AÁ5Â6	?5ȏ½ãÕ4FGL J0134.5+2637¿î8BTÆÀA oÞµ,À9U"¢ß"yÀ<
:䜸@@‰°îIõ?ÿ@7þtÆ?±:Çw"?šTg¥™H?ésñ~Ý֊@EZ¨6¿¸³ÿÌS€¿æÀ|ôGe¿ãÚpßf,…¿Ï‹Íþûô¿ã7a@6ÑοâV¢8¤Œ<AGNfsrq3FGL J0134.5+2638RX J0134.4+2638?ï÷k`9T?GÓ6§©g?Q)?Wýn?GÓ6§©j?ïú8mI?`¦€óû²Æ?G‹þJ؟?`¦€óû²Í?ïË!§AÔ?€Ëª/%}?zo,_ôJ?€Ëª/%~?ïÇ <æÁ5?k¿6"= H?|oጟe??k¿6"= B4FGL J0135.0+5338¿é¢V"Ζ¢À!^3‹GÇ?À;&ԅ'òÀ<´¯L¤@#hŸ§@Kj¿'zç?ԙ¨}b+n?æý6Œ"a@×'j@@ñ#
Ì?ïýÚ¡K¿œ¿Åz‡Á…Ç¿áû3¢™Èi¿ëß3םá'¿ïÿú÷''ý?ä™'¥RAGNbcuLQAC 023+053?èè+{³Ç?ÆЛ¾¯Ìz?Ïô_R0á?ÆЛ¾¯Ìz?ÚçTßø͚?Ôúe읯Y?âŒU™3?Ôúe읯Z?ØŠ¢ºv?¾¾'ñHÔ?ãøº®¢Äú?¾¾'ñHÔ?ÜÊzVåÅ?¼ØãÍ7¡?áùšÂԍ?¼ØãÍ7¢4FGL J0135.1+0255?êó•I§*¬ÀM½º
RiÀ;w³Š§àÀ<­ÓÀÜÕ@"[ÌÚ
Òü?ùYÝÿôB?ÍoÃ\`©
?´~!sBB?éSme^(ª@(â@Q~οïþš9҉¥¿¹³BVä?ïüùðòF¿Öצ$lpì¿ïé
?ƒ£Ž?ïгâ;ëAGNbcu1RXS J013506.7+025558?ïÿºz…$†?«KÑ>?a^¶Þg?«KÑÚ?ïþ4"¶0"?IO_D^Œ?,¶ÄœöÆâ?IO_D^ ?ïòû,å?Œ-'Yáʇ? šcNX?Œ-'Yáʉ?ïû§r7[X?BпÂgÃ?Ab7"'žá?BпÂgË4FGL J0136.5+3906?ìuŠzü®À6ðMDVq&À7´åÏxyÀ;<Ðjæÿ@"n×S9?øû"}ö¦?š›œÂݤz?´û0f…p@Õèc+Hƒ@uU6=SÈ?ïû!>>)0¿Ë»Cs¿×Ëw!ʀ¿ÑW8 ,ñ%¿Ö˜Ç¢"¿âCÖNUÎiAGNbll3FGL J0136.5+3905B3 0133+388?ï×@œÅÆ?z)!Ûy8?t_ö±Ô?z)!Ûy7?ï>+v?±'!ud.?ÜØ:'o?±'!ud.?ïʆ˜—:?˜Mtyÿ"?ŸF¯,íÏ?˜Mtyÿ€?íWÑ~aŒ2?¢6Ë£"?µAtóžq?¢6Ë£…4FGL J0137.0+4751?Ú:ÔÓ÷À,žß?–À8	wíwg@À;–ϲZZ¿@"58$t@'ßƤ"Ÿ?œºâ"Š;-?¹E6€o§@Ÿ
âµ@¹õ"¦î¿É8ÄA¸Ý¿àiˆ†a¿äªg|æÛl¿ã÷±j8X¿é!ÔfB¿ë|辚ÚâAGNfsrq3FGL J0137.0+4752OC 457?ïæVi-€-?a厯rÊ?i©–ÒÓ§?a厯rÉ?ïïÛ¾z<}?uP9á<¿?`$A…Áý?uP9á<½?ïÕ2ÆQås?veRľ"?ufœ×
FŽ?veRľ'?ïýôy¥?%Ó½ºÔ¶—?3x\7Ù|?%Ó½ºÔ¶k4FGL J0137.6-2430?î;)ö¸úÀSÒaAcwŸÀ9ɇî"À<BÎxžw@¿aj~#@@E®_ú?¨£,ëEˆË?½¨Ù'¤Þ@«c|§Œ@[òPêԿž¡{eQ¿ã2†óпçWã줩¿éž¥2¿êÌÝÿ$7î¿ïÿŠYŠµÑAGNfsrq3FGL J0137.6-2430PKS 0135-247?ïþÆÏÂ<€?"'¼$Ža~?#"Ü8ø?"'¼$ŽaG?ïü›B0?X·¸£ê:Ù??ë%ï'?X·¸£ê:Ü?ﶾõ]ˆ?"â^$­§?'PB¨Ÿž?"â^$­¥?ïÿ5jWÎü?J >ë>?Rµ w¿?J >ë>Ì4FGL J0137.9+5814¿ïA/öӈÀFïÃqÚ8À8Î3œ¾àÀ;ÊÖyù@ -ÐH'OÑ?þø–IƒÑ?¦ZßZÕ?Žà8±Ä«
?çé‡=G@úºÈ}Ü¿èQu¾sпԳµ'k€¿àħš
\à¿Ý
ˆïþ*=¿àÅ+<¿ØO*ÀH&AGNbll3FGL J0137.8+5813TXS 0134+579?ïþg[7G?"WìSžS?)ŠNL‹'?"WìSžb?ïýŒ´è
?Z(òø?3šX»—©?Z(òð?ï߉r@¼P?zv'Àp8Ã?p;Fß¡×ß?zv'Àp8·?ï÷œKÓÖæ?D49ºU?PÇhXR3"?D49ºS4FGL J0138.0+2247?·ÅbªiôÅÀCi:2?îÀ:%:G#«À<R÷eýŠÛ@²xà;"@}æOU?¸6Îs@–?q8áh¨E?ºS²ÚˆL?@z÷NU£?ì³åªê#ö¿ç^æªÄdH¿â ÿõEq¿ÖÄÀŽÐ軿äy-Œ*E¿ËgIû¡¡{AGNbllGB6 J0138+2248?ïþÈ
Ÿ?"¤p'3ú?#V"?"¤p'3š?ïÿ)Œ.?<­£?šÜNz<^?<­£?ïü"¸ÅM?>ÃÀ!ñC¤?>ï*9՘ê?>ÃÀ!ñBs?ïþ¿˜#•?yPO¨?$}Î&¯,?yPO¨4FGL J0138.5-4613¿í¸"/ÀQ0DR?gõÀ:j&Ñ%!"À<¤×%+3@îrì û@î¨|‹kÙ?¹õìUÔ?œ'Ý<Ü?ãªJè\?øs™)Ý?ïï
3Å)j¿¹ß#¦@¿çǃ·°¿Ù@X *,y¿à9¢cÑ¿ê	Ý>_SAGNbcu3FGL J0138.5-4612PMN J0138-4614?ïî€$¼[£?b€ØúÄ®ç?aÛC¤\{?b€ØúÄ®ñ?ïÉ~=©D™?Œp·¢H¦k?{@á+]³?Œp·¢H¦i?ï´m8ä­?ƒÃ
34»µ?'ä±ÿÔÂ?ƒÃ
34»¯?ï¦0,2:?ˆÏ"¤–LÉ?œ+9úy¸±?ˆÏ"¤–LÊ4FGL J0139.0+2601¿àώPA8ÀAϋ«`kÀ:´•ë/³À<8;-Ówâ@@,ôÄ0@"ÅDBO0?Í_á'¿'Õtß'¡?Íw,‡G‡~@¡¤ì³òá¿ë>øcSŒo¿à_*g²–Á¿Ûétƒ	µ6¿èBÜôb=¿àÒ\XÆ¿ïþ­…èÝAGNbllWISE J013859.14+260015.7?ïüÚD9k?<Ðk6¸`H?9/õÞ4Ÿ†?<Ðk6¸`>?ïþ=€L]H?KE¡å[?,'û:+Žå?KE¡åb?ïµû‹S͟?'‹ä"€ƒ2?'+—ÿ?'‹ä"€ƒ)?ïüYC72?/¥ž­9Žd?=5ç¦Foô?/¥ž­9Ž*4FGL J0140.6-0758?ë'mátWÀPäýó¶E¢À;¤ÍªB^À<™€'a–ô@ ÁŠ^"3N?ú¦¯ç¹¸?њ'ÇÅý?¢nªW¬å?óÝ­ûPm×@KŸ	0¿ìèiÿ#â?Ì:OMw¿×wS´Eí¿à­'f¿½›Á'¿êøC""~AGNbllRX J0140.7-0758?ïýћO[ê?0‡X±'3?1s%… ¬?0‡X±'[?ïþCf\|?U0íÀ,Ð<?.kɚ8>ü?U0íÀ,Ð.?ïÚýuMWa?vPIÁFY?rEYTO5?vPIÁFb?ïûP÷UåŽ?8Avÿë?B¼"¨iÉß?8Avÿë]4FGL J0140.6+8736¿â
ëø4@8ÉÒ¿UÀ:ҏØO·ÎÀ<A(¿<@ ï>fÃ?ÿy)L)¤>?Ç)×iÞÀë?¾ä0ì†ü^?ö®×ï?¾@
ç¿P7zì?ï(šÞ"ԿۏÔ>0<^¿Úõt,öƒ¿Ü/ö$_¿æ¾­OY§¿ÑHÈÆ­ÎÛAGNbcu3FGL J0139.9+8735WN B0126.6+8722?ïþkŽÝ?,óW͉˜Ã?.™Oç#?,óW͉™?ïýš3G"?L'}{|†?3/VeÃl?L'}{|x?ïõ´È¦—‹?c¿ÂfÀ\1?T–n²Ðëû?c¿ÂfÀ\(?ïðµfìàÏ?G²Ãì?^•2&>^í?G²Ãëö4FGL J0141.4-0928¿ÙÔÆaR"ÀQ1=Ùb·À8wŒE@ƒÀ;¯p"½'Æ@?mà-QÈ@²ƒ\@s? Nší¬–L?¨]ã#ë@ò*ڟg@0;'b|¿´#ŽûZÿ«¿Ý¡+>E[¿ãÓþð5ˆ¿âh·¿I~¿äàӟ¤Ë|¿â#*!;¹êAGNbll3FGL J0141.4-0929PKS 0139-09?ïýöáfŒ<?&ô;5¬—?0Hô˞"X?&ô;5¬?ïý¬DW*?P?ÃÊKÚ?2ßåF·?P?ÃÊKæ?ïà0诡«?pA1i½?oÏP^TN?pA1i½ ?ïÿº¾Y6¬>ùZI¸ø?Pi²U0â>ùZI¸4FGL J0142.7-0543¿âküyw-ÀPWÁ~ºñÀ;c1'À8À<±ÇÞP'Ï@JB•ü¬@3çÞ¡
§?Å?Ò(z#?ªqáÄ«–?äuòËd@Yï>½?ï÷®»iοä¿<Uñ¤¿ãʶ!œÁ¿è´¾c'˜¿Ëšã†!¿ïÿ~À¥L*AGNbllPKS 0140-059?ïþé…Îí¢?!Dtx+¡?!g£%ëÃ?!Dtx+¡v?ïþ¬Ùl'?=s™§~Ã?%>Ri7ìÓ?=s™§~"?ïè
W~ï
?q2î~Cp?gò¨òT?q2î~Cl?ïýª¾žÆ/?&¨Jϑò{?2ª	Ήƒ?&¨Jϑòµ4FGL J0143.1-3622?ÊîÛµÀRê–=Ć­À:Ìí¨À<"±ö‡±:@?þþMMf@qßƤ"Ÿ?¶áÓÞÓ¤F?»Æñ@Ÿ'g@.eÙx¬º@Q)¶1Õ»?ï÷XÇAr'¿åÀÇ`QN|¿ç!¼¿ænBÓº&Ø¿ìqT h«:¿ïþ–=Ć­AGNbcuPMN J0143-3623?ïþTëy»?'¯ÅìcŠ?*±GdRE?'¯Åìc°?ïþ"ÆÅ'?J¤<wï
?.f³"­›!?J¤<wï
?ïÕ«KÛ!?sJÈޝ?u*Zpo ?sJÈÞ§?ïþ¨ OÔî?>ß ~‹?%uû±!Ç?>ß Q4FGL J0143.5-3156?îg,"âÓïÀSköU\RçÀ;È~‰rÛÀ<´Zåÿ£º@Eöê,¯@E]D~µ?¿"/?]¸î¿·(p«¯Ç?öî |wJ?ýàÆúOçÊ?ìÒvÅY;¿æ2eByø¿çÅÅqŽ¹¿çš×Q‹
¿ãµíB
@°¿ïø:¿¯#AGNbcuPKS 0140-322?ïùm8ä%ó?C!ÍSTS?JKoh2j?C!ÍSTl?ïå\Ÿ?šµÒ´í@?ˆ†ºèÏX?šµÒ´í@?鷺Ü@¤ò?€{×µ"`f?†ÑHïÖÃ[?€{×µ"`h?št(?yÄ9g]ؖ?ˆ›™bÿ6
?yÄ9g]ؕ4FGL J0143.7-5846?Á¢ÌÎû0ÀL‰A|¢À9	ëîÑÀ;òˎkß@/Y®2'?üz}Å'¼Ý?¥%þþ^{?¦Ì7ógä@n:p>V@Çc,Ë2?ïüX`iLJ¿Ô["©¤¿Û÷cÏ2X¿ÜR²à£¿ßŒ.Â5D0¿Ò6ƒµ+ÆWAGNbll3FGL J0143.7-5845SUMSS J014347-584550?ïþ"DJJ±?0Ï÷
f¯î?'»»[Tä?0Ï÷
f°5?ïýSâ`H?O[DÁŸ?5cìýÁ?O[DÁ‡?ïå
ÀT‰)?sW‹x×Ы?jò?«vÖ4?sW‹x×Ð¥?ïùwÄhðR?9ë‡\½Žk?J î\>¿H?9ë‡\½ŽP4FGL J0144.6+2705?â'àà~ðÙÀA%ú](ÐÀ7¢½	á*RÀ;[.ÿÇËÜ@‡âÏmý@C`Ðԙ?•s‹½ãÐÊ?µ€À)¦@ â ÊæBÀ@K)<d_P?œº×+öS¿Ûü@Ã>®'¿âIÆ×p•¿áÍE˜…¿æÒí­íäu¿ç³Ø>ð֗AGNbll3FGL J0144.6+2705TXS 0141+268?ïí~©þ°?_!ÆmšA'?bæVNØ?_!ÆmšA‡?ﺖ‹äã9?–òqlp<Œ?Z]Ç1Œ?–òqlp<Œ?ï§nšó/?ˆ"ÑÉÓ?†$xC3Õ?ˆ"ÑÉÓ?îîuÃz9Á?ÅwøtžÐ?¡£È\cú?ÅwøtžÏ4FGL J0145.0-2732¿Öù#Ôî$ZÀS†KâCÀ9Xy˜rR-À<^ûE†@'‹öî´S@×EB<?¯½dác'?¸ÆÌ,¾Ïß@Ï¡·uM@ÉñS"ÒŠ¿Ø?$=È¿ä¦$Ÿòy¿ç»Þ¯¨Ð¿ê˜£?_¼S¿ífà‰Ã
¿î½Þ¨v¬AGNfsrq3FGL J0145.1-2732PKS 0142-278?ïþó'/óö?]Ý^t¯½? ÆÝÀŒP?]Ý^t°A?ïý'¼2Wù?LÎ
T÷?3jm@1E?LÎ
Tó?ïÁ'ŽJŒµ?{wêSØ1?>¸Ú¹¥•?{wêSØ,?ïÿú;?p%>ÃÜ:Û[>Ç?p"M>ÃÜ:ÚþÂ4FGL J0145.9+2319?êq a
Ù´ÀBì앿ðEÀ:ÏÓØZÀ<[‰2CI+@Ýyý@žÉý³ø?Ç·.jv–_?·jªÃ¸|?îzÜ?0—x@8'ÁÞÝ¿ã7=N?(4¿½x³š÷'ž¿ç=Fý•lŽ¿çLƂ/ð‰¿àɺ^5?}¿ïþP§ETAGNbcuTXS 0143+230?ïùöÆY³?D1ˆäW†4?H$曱9¥?D1ˆäW†4?ïü‹u
«ð?Xã×£ þ?;¤W' ˆ?Xã×£ ú?ï³fÞTVq?€c͎.¹Ü?ƒ&HjêcÅ?€c͎.¹Û?ïí½ JJ-?Qª®l:	?bBßµµÔ?Qª®l:	4FGL J0146.0-6746?ï¼ÈÒîÁÀHBòù‡?ûÀ:$"çƒ1xÀ<"Ö«rßñ@#¿ÆÿÙ??ÿD¶Ê,	?¸\ǁ3qG?¾E¿&ñÜQ@·Üz¿¹¿@|š	Öîd?ÚÀïÿÕÙ¿Êèà©£}¿Ûú©ÿÿáр´¿çÊäÊðS»¿àów[0AGNbcu3FGL J0146.4-6746SUMSS J014554-674646?ïüñ"e°?8'rí¦ÑŒ?8qëdҀ¯?8'rí¦Ñ§?ïý"0¿p?H©‰ã3|¢?3^ê€f?H©‰ã3|©?ïÒzŽM9`?xžóÌêw:?v¸ÙcOö?xžóÌêwG?ïô‰¤0ï?DTÍ2n¿?Ví"é?DTÍ2nÅ4FGL J0146.3+4606?å¢Ì¢ÍօÀ/j²[1~þÀ:ʄս6WÀ<"Ä'k§ï@VÖüPž?ÿå€éŸk?ÇD×àÒ\?Çaá†îQ?ý¹áˆE´??û™R.v
?ïäY!bü¿Ñ²mÛ¥­¤¿àQøPV¿âÌÅ«p[³¿ã%™'¥R¿åAmž%øAGNbcuB3 0143+458?ï¬6âK¯,?'_Ü>ƒFý?"òGm5
?'_Ü>ƒFþ?ï])"Z°è?§'oµEÜ?"Z͔©ã?§'oµEÜ?ïªrT?•{÷J<'Í?žj¬Q¼µn?•{÷J<'Ñ?í$ë!J?˜ŒgÛÌDä?¶Ùâ¦÷5²?˜ŒgÛÌDä4FGL J0146.9-5202?Ô~8²¡ÀO~÷üü?À:aØ›ïµÀ<!Õ<Ý×@h <K	ê?ÿUûµ¤a?À®I)ʍ?½>[/{˜¨?þ"T8fxÛ@P×8`™ž¿ëc>Ò¤?ÇA»Y¿á»Ëǔ¿ß¥áË·y¿ÞËSûÕ£á¿ïô`{?çAGNbll3FGL J0147.0-5204PKS 0144-522?ïîŒq´ô?a í&ç?asŽKÿ?a í&ß?ïêCñ?vïãƜúJ?eþ¼€î8?vïãƜúJ?ï§
þfˆ?"ÑáM±o?†<€f]ûW?"ÑáM±l?ïs«ó+ë9?~$d´à›?'Šš'™?~$d´àš4FGL J0147.7-1321?ïŽ6Ù	ÀQ½×¡<%JÀ;i™ù:éáÀ<ÐI4&x:@Ë{uÂ#ü@Œ¶â¼y?Ú#<E*¬|? ú¶j	ß?Ä¦ý/k?ÿÀN²º¢?ïú
'Íx¿èå).‰¿â;¡–¾¿Óšß_ ¡á¿é~lLYtæ¿ïÿúŒ"¸'AGNbcuNVSS J014804-132019?ïýëí³l?4çó{º5?0 'dŸ¯5?4çó{º4î?ïç$¾ñœ)?}
oÒ»<ú?hÛAc×µ?}
oÒ»<ý?¤K3?ˆ$*Ó«\7?–í3?µ?ˆ$*Ó«\1?ïëápƒÑ?TÈÎcO›	?dã|0:?TÈÎcO›4FGL J0148.2+5201?ïY¶ý3³À#¾åGÆÀ9³EB<À<!»¹@ ¹%ô†O:?û^SEÎ@?´lŸe‹u?¹—½÷FóÚ@Tù¯ƒç@FI»_è¿ïýè~;?ïÿõÿ 1#¿Ä")Èü3¿ÜX
Ã}m¿¿Û¼ýÌÉó¿ÕÅi@¶SAGNbll3FGL J0148.3+5200GB6 J0148+5202?ïüµ¨
»‰?>¤ß?:R¿'#½&?>¤ßG?ïÐ"M¼Ÿ'?'­H°†	?wîÙ!°>Ð?'­H°†	?ï¶þ28zÂ?ƒ¡í¹?'@sqáO'?ƒ¡í¹?îÑF'õŸÏ?'wiiÌ&¾?¢ë–à¦?'wiiÌ&½4FGL J0148.6+0127?ïºrao¯¯ÀM"!ÄuæÀ:q'ùCM]À<e€<ÑA§@T˜Û-¸ @Ê¡C²x?·­®¤m³¿­Œ^Æù"?öq?|Ì@Ãú³ºØ?ïzÁҝÇ&¿èmÎÜd¿ålXï
¿àæY›|Ȩ¿Ù¢†,Ù¿ïú?̞©¤AGNbll3FGL J0148.6+0128PMN J0148+0129?ïýçȖœµ?-ß7ú?0Á»K^?-ß7é?ïüõxދ…?R"!#ـò?8T9£Ö>?R"!#ـø?ïïw•–ôT?fÝÐ@®š?`ˆji¬·?fÝÐ@®¥?ïñÒò·~?Jú0›$õÉ?\[þ'8?Jú0›$õ·4FGL J0149.6-0734¿ê¥ueïDÀP… …±…À;L;æ`ÊÀ<§Ö»cý@Eûxö@Èïþ*<ê?ÒEè8¹?ÃØEç?ê§?ñ"ì~Bûþ?úü,ý~?ï³@S'D¿Ë»5À¬-¿èåTƒ¿ãÅ©!ÌÙb¿ïþ
¡ÿÏ¿ìRÍAç«öAGNbcuPMN J0149-0733?ïÞay¥;?q|«[O"ú?pÏC-bxf?q|«[O"þ?ïSsl,m?§ç›Np%?•'œ2zr[?§ç›Np%?î°î	ցš?"«ÑÚd9'?¤ñb—æj?"«ÑÚd9?î+"æV'ó?–G"åÜa‹?­G±š–ÐÆ?–G"åÜa‹4FGL J0150.6-5448¿ï_†!s2ÀN%db€'ÙÀ;K¹Z)ABÀ<ëªfpw@ #Œ¤ÄS?ùÃԅþ²"?ÓñýwŠ%?Ï*y¦41¶?ôm3	AÈ?ýî¦un¿Ò‰÷Dðtó¿êÖc"3ÖÇ¿ßü^ Ia¿Êç‰¼'¿çÕT{ç¿Àψ=üÞAGNbcu3FGL J0150.5-5447PMN J0150-5450?ïúþŽà¼þ??DzgÂÒ?DÄ}t??DzgÂñ?ïù=š/ñ_?_ƒÝ i³û?K	—@:Œ?_ƒÝ i´?ï§0'–h?"g4̧?†3ۚeÜR?"g4̧?ï߬'Ñ2?_9qlµn?p)ì~f-?_9qlµn4FGL J0151.0+0539¿Õ3µ»Ý*ÀK—þŽæ¸À:Á'ï2RÀ<mwVx²™@ӀÖ)Aî@ßûH
ZÍ?»ϘY'º¿²à#–³
Y?øq‹'æÎ×?þRP6ú*?ïú¦$¿ëÆíàBËW¿çt‡>.¿ÒbÌéR>'¿Ú§½ž±†u¿ïÿülòAGNbcu3FGL J0151.0+0537PMN J0151+0540?ïùz¯-&?C˜‰‰ŸŠk?JC£Kq:?C˜‰‰ŸŠ]?ïÜèÇ
OÔ?ƒRÀ!è?q‹œzØÔ?ƒRÀ!è?ï»DÉ'š?€PÓëHmo?>nͶm?€PÓëHmt?ï£DZø@q?uß76'®ð?‡.éAïã®?uß76'®î4FGL J0151.3+8601¿¥gÏ6Û´@7GM3H,À:´4çhÀ<h23Xòà@b¡…vL
@BLƂ/ñ?¶ ß´*·?‰0QxåçG?θÐV<<@Ee*§¿çIpŒZ¿áoáÐêê¿çÞl²[¿á['§åŒ·¿ç;ØÞ¨íJ¿ØÖ^¤ÑAGNbll3FGL J0145.6+8600WN B0140.0+8546?ïøP"]Wì?F­*
±™?N½îŠ W?F­*
±¥?ïýÊl{l÷?Iå˜`Ð×?1¬œ$˜M[?Iå˜`Ð×?ïð—'v?dô
»lŠk?_øÐûÙ¥?dô
»lŠj?ïö`û[ç?Có6#º?Sé>	H1½?Có6#º4FGL J0151.4-3607?닫†C–EÀR™—_,¶AÀ:Õ,D,À<Â(äû—»@ʆXõµ@ü\Wë‰?Áú"³Ùa?°ÔâšêQ˜?ïœÙŸÄ @ AO€›Ç¿»,€¼}õ#¿Ü|؃9Zë¿é§¢pØ°¿ÚDí$±W¿ê>ku™à¿ïô¸~Œ"
AGNbcu3FGL J0151.0-3609PMN J0151-3605?ïØçÞAuä?q»Œ×ó?sŒßE
–?q»Œ×ø?ï×Ó´µ[?†2'
Ò?t%ý%S?†2'
Ð?ïÒL'Ì6?‡ÖLü"Â?Œ‹lßLòk?‡ÖLü"¿?ï¼GªÌ?o£…ä;À?€î•Lù"?o£…ä;¼4FGL J0151.7+5455?íþÔqœåoÀÀJÕÀ:{93'uÀ<)'(±Ïñ@x97Úû@ßçžà*x?Îû"áN?ÎgΛYa?ñ"ÒTÌ
/@ô"µÜÆ?¿¾HyìU(Q¿»äqY3¢ð¿ä&&À^)¿çO[½•ø$¿î,¦AÕÏ?Ø_`'÷–¥AGNbcu7C 0148+5439?ïi
y8uw?"™XrVõO?'ÞPØñPú?"™XrVõP?ïûMá"?^º#Vÿ³?C—öÈy°J?^º#Vÿ³?ë×Д«ö4?©ˆ·̹?À ½­P'0?©ˆ·̹?ïÐz$Ø»p?f2¾Ž¢ÒV?wÂ퓢G¬?f2¾Ž¢ÒZ4FGL J0152.2+3714¿ßeÉáBêÀ8Sü–ÿÀ:¶ÁȌÌÀ<†xºüÀ°@‡r¨¾û@e%îÇÉ?»üžw?³£çÑ5Z?ñ¯Nìő@ކÀùÚÍ?ïBUåæ¿ãã/áD¿æ³û¢n¿áêP (êZ¿æ:D4w¿ïÏöbreùAGNbcu3FGL J0152.2+3707B2 0149+37?ïý«É¹¢¹?*•QSXÇ?2¡²2ê+?*•QSX°?ïþwï 1þ?BR¢PwJ?(
üà‡?BR¢PwIû?ïò9í	=?bF…ö1B?[Œ%íɆ)?bF…ö1L?ïïð4ð˪?I¶Ó9à$í?`Ë4U–?I¶Ó9à$æ4FGL J0152.2+2206¿îo[»®GÀCM¶¡è´À9²j²üA/À<7Üýœxq@Üωë|@åO±;?¶Y 
ý?¾µ9³*q@+ÞàˇR@[Õ¿É¿³Û÷žBÜÛ¿æOâ+ã	¿èÞÙ	1µ¿ç'Á†¿ïÿùµc#¼?êL»P£‡AGNfsrq3FGL J0151.6+2205PKS 0149+21?ïþ_9ÚÆÙ?-™Â>­@f?*bS'z?-™Â>­@…?ïðTš9ã‰?ã+H'^?_Vˌ8ò??ã+H'^?ï¿/â«?|"Ƕ",?€:´U>¨?|"Ƕ",?ïæŸoºÇ"?`
ȳ"7M?i`E8l:?`
ȳ"7J4FGL J0152.6+0147¿i‡X˜}¸ÀLÅM@$³>À9mRj0'À<tBÇü@%L=gµ?ÿñ|D=?¯Çˆ"9¿ƒgáfÝ?Ôi,"AC@	B1}Ñ?¬¬j_Lõ/?¸I*ì<ԝ¿ár]ëm¡Ä¿Ü"í*¿à¢¸'¬eN¿ÓVPn­\ÅAGNbll3FGL J0152.6+0148PMN J0152+0146?ïúÝÃ
-???c04ß?E¼ˆóËKi???c04Æ?ïþFáë"?G¿Ú¤àVü?+'îQMáÍ?G¿Ú¤àVß?ïðÜý–áÈ?eòÅæŠ?^FÒ<m™?eòÅæ'?ïù±€`e?;Nøÿ´Ã?I;¡þ~j`?;Nøÿ´Û4FGL J0153.0+7517?Õ-Pèhn7@)É%x_.À9û)=+ÇÀ<L"4­†¶@ TB…Þ?ÿ&ò³c%?·—MŽÿä?±BZÃpÆ?øln¾#¼ž@$ìH`¿èK·ùÖñ¿­Wåš#,¿Öþqàm¨¿à(l/Ô¿à{'{üP¿áÍ´ôhó	AGNbll3FGL J0152.8+75171RXS J015308.4+751756?ïâÃz	]¸?i…ÄÁš%ï?m<…ö¢G"?i…ÄÁš%ì?ï¯ a4¦?šÍím£ÝÅ?"7ç¹rÖz?šÍím£ÝÅ?ï±+6pd-?'—X[?ƒµ2cæôš?'—XX?îCµ¨Ö€?"Q‹¡XÉ?«Ä§år—ý?"Q‹¡XÉ4FGL J0153.4+7114¿ä]+ŠoxØ@!ò!ȧ¤À:jfóT À<O$V ž@!"U©€Â?þuêMT?º$ëFàd.¿'y(_ð€†?Ú©=;äó@:šþsì¿ïûÔ¢.=«?ïÿIŒ;F¿è€§?tŠ¿Õrü øH&¿Ü­ÏÜv¸ï¿ß{"¶
nAGNrdg3FGL J0153.4+7114TXS 0149+710?ïýÎ>ϗ?-½T¶yl?1Ž	ƒG8?-½T¶yy?ï÷¢lãaZ?ldàñ $ª?P»&9=LL?ldàñ $§?ïë0pZ"'?iëìôU;©?dϏ¥{Ú¹?iëìôU;¥?ïÓsŒ½öÄ?ixyŸ®ùì?vF9¡ž7?ixyŸ®ùè4FGL J0153.5-5107¿Ç"V*ׂÀO¢sÿ¬*À:Ìg¼§»›À<z9ŠeI@üÖ~|\È@
goF	?ô¹©š¿¯"èÁu?áèæ€Äa@øªgr*?ïøs^œm‰¿éú÷k¿éQÃA2Ð7¿îݼ¾â©X¿ïý®aQԉ?ì!1¾iÕAGNfsrqPKS 0152-513?ïÿÚhè3?'˜Ì(gK>òË¿æ'|?'˜Ì(h?Büe?¤‰…æv{—?ŠU¯@ýæ ?¤‰…æv{—?î"ý`ßÈA?¡ÕðÑ©4°?§°)ò{ç?¡ÕðÑ©4°?ï億KM?l(1àa˜c?j{{´²ïD?l(1àa˜m4FGL J0153.9+0823¿êï<ύráÀI°·ÃPLIÀ8ðÑn=À;ª¾®&@7ÕÞCl¼?ý%'6¥®{?¬ÐZ¿6?´s"·e•@Jñ£EêÆ@BíPøì¿Ðmâ;sôn¿ÕŽ_©³Ã¿àlâiø¿Õ¥^~~¾¿â1úï,¿éäÞq9þÿAGNbll3FGL J0154.0+0824GB6 J0154+0823?ïýaL'Å?0ÂØhµa?7"õ›q׶?0ÂØhµ ?ïô©LÞçŒ?Œz"f¹ç?V­fB0èÔ?Œz"f¹æ?ïÈ»H¥¹*?€$†Tæê?{¢[­#kƒ?€$†Tæê?ïí.ˆ¯¬X?PΓYîx?bÑwPS§¯?PΓYîx™4FGL J0154.3-0236?ïì¾£Gà$ÀNž¢×/ýÀ:ݤÌӂÉÀ<œ¿eÛüë@| ®vJŠ@É2¼î¥?¼´ßWD5¿©P>Ü´¡?ð¯¢ðZp@Åôw‹§¾?ïíYx0=¿åföyn€ç¿äìÔ	0'¿â!ÛA¯¢Å¿Ö3~݀¤*¿ïÿî,˜å?AGNbcuTXS 0151-028?ïþú݁A? "iÕf¦? _2'ëòí? "iÕfx?ïü¦rú\^?SbɁÓþ?:Ìh-"?SbɁÓ?ïðØcr¢­?hCàãQ%ž?^O9º§	?hCàãQ%"?ïðZ–æ?Oà ¶ÚS†?_ÅKÆÒ6t?Oà ¶ÚS4FGL J0155.0+4433¿í´Çn*'âÀ0Ú©÷µ®£À:b-—è¿rÀ<C8d@…"†?þ]Ã_eÁ%?Á ¨A'<°?Ós k°R@"¡ô±î@žWˆ
€?ïù$¯ñ¦¿ÓÄÐo½¿ÛÖ}»Áã¿ç2BÝË!Ò¿æ\¤¡	¥p¿Ü9G'RAGNbll3FGL J0154.9+4433GB6 J0154+4433?çº{ì6l?Å!ûÔð]G?ЋÄ'"&?Å!ûÔð]H?ï ÂÒgO^?¬.É!óú?›ç¥³5?¬.É!óú?Þc#Ÿ`?·Øú-'?àÎpn0tP?·Øú-'?í˜oFy?š¥fºÖßW?·;<‡ÍÌ;?š¥fºÖßX4FGL J0155.4-0625?ÓÉùŸ.ÚÀP`,'À:óÀƒé.,À<–'Jÿ†@r)0zò@>
í(Œç?̇œ–ú?̇DÒ»?÷¾XzëX©?ÿúa÷ì¶?ïþ\AIvl¿Þâ˜[V¿ç·y^:ÈÔ¿í¾I¡ßŽE¿ÕÀŽeˆðÕ¿ïÿ5jE8AGNbcuPMN J0155-0621?ïñ¾¢2?hëkòå?\'޺ߛï?hëkòè?ï´Z–©8?'†(ºÁ×	?'é~ÚU²<?'†(ºÁ×	?ì‹Ã`©?«¥:øÎd?»¡çgDúµ?«¥:øÎc?ïVû¥?†;•S°ÇÉ?•<¾| ‹g?†;•S°ÇÊ4FGL J0156.1+1502?æÆÈNÉöEÀF€.#)À;›ªgG6öÀ<Æ´!Û@!w©úå¹Ù?úk³\¹>{?ÕT¤òé?ÊÑ(¼Œ¸¶?ööc3«þ÷@gÙ¦¤ð¿é'æ!1¨ï¿ð?ð¿ÒŠ…¼¿Ü8Ʊ•¿Þϑ7ËHhAGNbcuRX J0156.0+1502?ïý@G@ÏÜ?,°¡aÔ?5ýÅù?,°¡a}?ïýÇO¹$H?N"Õ"Öè}?1ł6ݸ?N"Õ"Öèƒ?ïݞ,ìE½?p™‡aýx?q0é‰Ý!Ö?p™‡aýp?ïö"–Q"Ï?G˜kCjRH?RÖÓ\Ø_ç?G˜kCjRH4FGL J0156.5+3914¿É™\
®I™À5èÍJ¡À9ÒU݂&¶À<djQ­q¾@áaKI{@wí"Ó8ø?²jËOõ?šµÉƒŸºÎ?äBÎFIm@…䀝Ÿ8?…Ñ1½¿â'Ÿ¿ùTÀ¿çÿF!!Ä¿åHùn‡Q¿ä_ÞÝpˆÿ¿æyi"ƒb¡AGNbcu3FGL J0156.3+3913MG4 J015630+3913?ïþn…p	´? ¶µ·Cτ?)¨ÿdÀr? ¶µ·CϘ?ïþQA½Û?Ef›ÚÐIþ?*æ+ä"WÞ?Ef›ÚÐIã?ïíÏC‡—Ì?cbX·
·?b0¼xh2ù?cbX·
·?ïÿmÿðâ?C
.Åøê?PãÓB?C
.ÅúÇ4FGL J0156.6-1758¿íäs{"°ÀRÓo~=À;NÞÚ‹À<łw>$ÿ@Cl§s!
@EÜ@W?ÅøvHܒ¾¿«—s#¹¹?ã̤ˆàä²@9˜¸=S?ï8ßî°L¿êˆH8}õÏ¿áÊDAxpT¿ÙGőo(­¿â"^~»qܿﱺ!Ï]¡AGNbcuPMN J0156-1800?ïø°È‹h?FÝ`@t$S?M<ÝÓú^b?FÝ`@t$Q?ïýuGèö?Hí‡kŽ?4WÍÀ¸Tr?Hí‡k?ï×þ8nIx?v—'!ç?tãÈÛD?v—'!Ý?ïöÙ‹£,?DBèz Ö×?RÞL蹦q?DBèz Öþ4FGL J0156.8-4744?ánšÊ`õ¥ÀPp@ ÇÀ:mDù.T§À<ªfÄZ7"@ŠÃvˆr@Õ~œ¾H?¸´XaÀå8¿›ûÚ'ö7?âa0œýç@	i°|ʬ¿è6úhŠ'¿ãe—=$¿æ
5bhß¿Ý2GZ²~¿Ýw¼Ú¼N¥¿êNHÝêVvAGNbll3FGL J0156.9-47422MASS J01564603-4744174?ïþa;:á?#{ûrüÒk?)ã$QÏ´?#{ûrüÒ?ïþ˜[ç•?FNJ"è21?&zF!†«b?FNJ"è2Q?ïøR3¸Åõ?[)•ù?N·1è/£?[)•ù"?ïþ¯öÓ9J?\"€>ui?%'Ìk]‰?\"€>uÇ4FGL J0156.9-5301?ëqÙX¤™IÀN°å^³À9Ü¡|¼êÀ<³†ª©Œ@¡ 47?øת@°Ê8?´->§…–?º¶¢Êê@F"Ú8+@‰qü­Æ¿ïáâ"Ÿg9?í…ʬk-?¥G´t'Ln¿ÖŠš"U•¿â3EaÞí6¿ÂèÛùe‡AGNbll3FGL J0157.0-53011RXS J015658.6-530208?ïþÝsè¸W?"y
%VM?"(ÁtzŽ³?"y
%VD?ïý‰"Ëþ¸?Sk˜º¬?3¶é 
Ho?Sk˜º±?ï×ÊÓ<z½?wã5жeú?t–a¡6?wã5жeö?ïüf7C¦©?2úzbî?<ÎEâÊ´D?2úzb4FGL J0156.9+4648¿éua‡üôÀ--"n)ÔÀ:ë<©Ôz@À<h-æÃ@Ÿñ‹¡´?ÿ–îú>¯?Ðy<¬Ù'?՞9¾g¯@Xä1ò@þíï]'?ìç`vã6?ï­Ù¢H>Þ¿Öl|ªöc¿çˆD§Ï½B¿âtÒ9ô¿ðAGNbcuMG4 J015651+4648?ïÔuZÀY–?vH¶Vö?uÅRŸÓ4³?vH¶V÷?ïÀ´ôä]?—ßa*Ðûk?¥…ñ
Ñè?—ßa*Ðûj?í'p0®l?¢ß–íJf?³ì~zŒŸ?¢ß–íJg?î]M׶?—B!l!Ó?®:'+""¶?—B!l!Ô4FGL J0157.7-4614¿ì.ç|ïzÀP´˜5‹'À:LvѵÀ<!4x­Ç@ˆW+µæV@ê}ík¨Æ?¿à	ëf?û?ÌꗸîÉw@–l£—I]@A	—ÙP?ïü=¿ÿ	¿Û==ÛWÕ¿åÒ¾^"¿èÛ¾WîÔ¿íþ˜ ó–¿ïÿþR€ÖTAGNfsrq3FGL J0157.9-4615PMN J0157-4614?ï½
ú ?H?"ä*ý\%"?€½Awð.\?"ä*ý\%•?ïûƒ?ºº-?aw«ó'j?AóKr?aw«ó'q?êú˜7sÄ_?«Gù3Üħ?ÄŸ"0îƒ?«Gù3Üħ?ïø?²—¸??´)ÑÝ@?O5£Ñk??´)ÑÝ4FGL J0158.5-3932?Õá vkNüÀQÕQ֌i/À9‰'TPº-À<L~D©}<@îJ µ'-@LQj‹?®p®hß?®¬ˆ×[@Gjdø¨@ÝÍM{2ü?íŽ:‹I¿Ý—Ä{Dš¿áž¾fØ|-¿ãâC çU¿á^û}å3 ¿âaÈýŠYáAGNbll3FGL J0158.6-3931PMN J0158-3932?ïü'5z?5Xh©ö,?;w¦Wdã?5Xh©ö	?ïþz›9j?D¿Û®¦Ì?(VLg	W£?D¿Û®¦Ë?ïãÅ¢±w?rb‡™½#?l:]Nˆó?rb‡™½.?ïút߃ö?64+Eð€?F,ƒµð'³?64+Eðn4FGL J0158.8+0101?±=^9׏ÀLÁ¥~ª*À:MŒuĨ;À<W#I±$@.û%OÅ»@d¤Ú¦?µ3>ñ­V濱*óÄa?úõ³;?ï™"/¢&}¿ã·M>w4¿ßêvjG¿éI­=ef6¿âò|Ÿ7é%¿áa¢
×I¿èËRä©bdAGNfsrq3FGL J0158.6+0102GB6 J0158+0101?ïÃÆnx‰?'Dg€ Ö?~Èû7¼?'Dg€ Ö?íÄ	W?À]¸ã=
€?±ßµG¿w]?À]¸ã=
€?î|²Æ^ŠP?žÁ§ï؎!?¨4ӚZë?žÁ§ï؎!?ëûõÊ P?¨1—Þ-Ð?À˜(×~½?¨1—Þ-Ð4FGL J0159.3-4523?è˜WèÌ
ãÀPÒt>–=ÅÀ;ûAT^&À<ZÁ#>@ƒ+̱º@ñÀoz?ÃïÊhC‹E¿­Ähœ˜ôÐ?çM}å-@
·y
²ñ?ïÆ­czù›¿ëϚ!~ÕÉ¿ââ΁WÙ[¿æÿ¢!¨qN¿á¬Yûð¿ïÿýç!éAGNbcuPMN J0159-4515?ïÿS][ä­?¨0aÁpÎ?"Tƒj_­?¨0aÁp0?ïþb¹
¼I?E7yÍ1K©?)Ôo$;ys?E7yÍ1KŸ?ï×ì1£2˜?wq¿å›M?t	ç.f´?wq¿å›C?ïþ6–Jê?!

z.8\?.¬–›QuH?!

z.884FGL J0159.5+1046¿Ý"ÃM‰ú‰ÀHSπÜ3rÀ99I—"ÇÀ;ù'ì®@¹O"ðB?ÿa,:=é?­ÊÞW†? ¥ ÛN½?ó(᠙h@Aàz~¡F¿ÝèÀž@Gn¿Ý/ò6ᄿà†=~搿áüŽ''Û¿Úª-e"؏¿ÛLáD¨ücAGNbll3FGL J0159.4+1046RX J0159.5+1047?ïýÔ%[(?)71µ¤ ?1^Ô&Àj?)71µ¤ ?ïþ|Ã8?G—õx'­'?/¿È3̇h?G—õx'­?ïîíÀ"½n?k±¯þ#á?a?ÝBø?k±¯þ#á?ïü-•÷?1ðŒÒý??‡¦"PC÷?1ðŒÒH4FGL J0159.7-2740?áÌÔü[ïÀRµ;Ÿ_À:"z-ëÀ<ÍÄC'O@È÷C«@
¨_/:€?·iŸUñ#?±]CRAf?÷Ê	ÞÒ@È7Zµ-I?ï÷"_mλ¿Ú]&š¯™¿àÁÞây|¿àÂÞZ"Ê¿ââ½ÏÚ¿æÑT¼÷"AGNbll3FGL J0159.8-2741PMN J0159-2739?ïøe+•?Pgl"D§?Nk·S©/?Pgl"D¤?ïúŽTïJS?`pc	~ÿÝ?EƬBÖ³<?`pc	~ÿá?ïÍoÒËn?€ÃÆkÑDç?yHu–šI?€ÃÆkÑDé?ïÖöŸT¢?c\
Ù¨Z?tö"°U®Ô?c\
Ù¨^4FGL J0200.3-4109¿Í3\é'©ÎÀQ"Ó0"'À:‡4–àµÀ<'oQÇrñ@ p6åDgä?úéQgÑ q?ÁblÇ(ž?Áۛǜ6W@)ý¢W®=?õA÷˜(«¿ïÌ7Z?åéáæ9…]?£ûüÞпښr¦æ‰¿ßGH~sùL¿âÒ*AGNbll3FGL J0200.3-41081RXS J020021.0-410936?ïÙÕºþ f?tŽçÿEœ?s"€¯Ìb?tŽçÿEŸ?ï[J
:{?¦ÒV'þ?"–¾¸°A?¦ÒV'þ?ïŒáAOžB?ŠTîûØ!?ŒÇ¯¬oy?ŠTîûØ%?ìå°öó…•?£!Ëކ?¸ÒxHcÓa?£!Ëޅ4FGL J0200.6-6637¿í¥MܝG9ÀHŠÎóÀ:#8ê,YÀ<…6žË2@@zž×œ	@ÐeÁ•?³î`¬ßX?'dmÆ_¨æ?ÙiôE6ÀÜ@pXËô
¿ám‹zÖ¿ä'z¡†Î¿çúVÞ3&ž¿äUûŸž¿é±Èd¿ïú3¢Ä»†AGNfsrq3FGL J0200.9-6635PMN J0201-6638?ïý½Ú«?_?0¨R'Wu®?2*¦?0¨R'Wu»?ïþqßl??DJØÀ«Æ?(â	<Æ?DJØÀ«Ñ?ïãrŸ|ó?oöÃQ·³A?là`ƒ¤?oöÃQ·³@?ïþ¹}ü´?³sWa?$h 4¿‰?³sWŽ4FGL J0201.1+0036?ïr݊†ÀLÌڐî¢À;~eæä¦À<ÆCnÙÒ@!4՞'?ý4¥ùú-?Ñ"×ü?®-žÁ0?ßŐÃ\5¶@‹ìé͹‡¿ïL³'#i?ít來
 ?ÞF}¯y¿Øá<O¼¿Ýü"C¿‹¿àqS>ìNóAGNbllMS 0158.5+0019?ïÿÊ·¦ó?Ûùiq•Ž?F©!iÄ?Ûùiq•;?ïü¦IK¬?YÝ\"ŒrV?:Í·¥¢•§?YÝ\"ŒrM?ïï!¾§ëë?g'"_ïÊ?`ÞAX°?g'"_ïÔ?ïöi—Œ¿?Fj…7À?S,Ðç΄}?Fj…7Ï4FGL J0201.1-4347¿î—šêäpdÀQóà7ÝÀ;­†)zLÍÀ<ïÈN¸Ê·@!ñҕ¹?úÞ@'—?ÑV€[¯ÿ?ÇZHJòlš?÷žçf¬"@4•¥RÝ?âÖtì;'?ÎR	!¼¾7?åǂ«@‹¿ãæxw¿¥™ÑÞë™}¿å²?'ÌÎAGNbcuGALEXASC J020110.83-434654.8?ïð²eDvƒ?[#øv"«?^›5w÷¢?[#øv"?ïýÖäÎ<}?JŠYÄFX?1Hَl?JŠYÄF|?ï†Þ C'?‡ÇÃÄT!÷?ŽxˆWï˜?‡ÇÃÄT!õ?ïö4 AÛ.?Jåê>ß ?S—¿|I¢u?Jåê>ߔ4FGL J0202.4+0849?ïvO«ˆbÀI0ߛÜjÀ:Ðè¨ËeÄÀ<tíSUª@ õ.vŠö¿?ú'4Û©ß?ËÏö¸X¡'?̸Ž;íkÿ@H&	@Êúmnî?é¥C†g®¿êâàíB¿º¤›?áíE¿Êü¬äOx¿Þ1¯$›?â¿çJ¼¤¡5AGNfsrq3FGL J0202.3+0851TXS 0159+085?ïüÔ­\MV?@af°ŠÝ?9Z••K»?@af°ŠÌ?ïúÞ.{­O?\¤Á,Gô?D‡FJÃ0?\¤Á,Gù?ïÌ>ñ6ÅÍ?x='Ì©?yà‡d»?x='Ì©?ïÐ(Šˆ'Ë?gnhg/?w뺻¶šþ?gnhg14FGL J0202.6-0258¿áâïÅ:ì5ÀN9a€M˜9À:sëLÔÉÀ<cݯs²@7súž@óI¾ó(?¿L͹ð…?œÒ¡^E@ã?ÜðqA¶®¨@À¿aKæ?ïóÒà¿ç1e}³4¿ä͇§ÿê¿Þ¹%˜b¿ïÿÍ?¹Ss?ïøŸƒ¾fAGNfsrqWISE J020239.94-030207.9?ïçjµÚ©J?g]îï$Ib?h•J%V¶b?g]îï$I^?ïêâyçâ?|¨ƒ­ d¿?e†ì²?|¨ƒ­ dÂ?ï'÷Ãœ€?‰Èô–›â?B?XßÂ?‰Èô–›å?ïå'OmÀu?^t)
¤s?jØ°'?!?^t)
¤}4FGL J0202.7+4204?År"‰EǍÀ2ÞD""N×À:¿í½qæÀ<ŠÊ'_éu@ŸøUӍ@ª‰žyÓ+?ÅJ¢Ô€Ë?·ßT"@X?òΝ‡dä@M>ê¡t¿éæÓ^6l#?îß¦Ä$ˆ¿ædèÕ.›¿ØÚf}ãZ®¿å¨Ñl×Å¿ïþÖj€˜AGNbll3FGL J0202.5+4206B3 0159+418?ïÿ$ß
"? E§?ìW?䯖}? E§?ì"?ïýÅð¹6?UsáfÀEc?1Ðz7GT?UsáfÀEe?ïíÇÃ=?fJvX?bp8û<Ãr?fJvL?ïø¿˜ôa1?>h´<-ê?Mœ.{>»?>h´<-Ì4FGL J0202.9-0225¿ì/¾‰‰|ÀM÷Õ<ÝÖàÀ:Ó¡ÏɏÀ<|%ä–.@ ÈAÒt>?þŒÇÄOOÉ?ÄÊàä[ߥ?AB g"×?þp'Ldë¿ïïê^-1ç?ïá¢!¨¿à:r•;¿Û907Ö0#¿ê—Š@
\$?ÙTÎäT'õAGNbcu3FGL J0203.1-0227RX J0202.9-0223?ïøNÇôn·?MŸÁ›…/?NÄà.E%þ?MŸÁ›…%?ïñ¬±Mœ?w±)xÇ?\§ÎdÆo?w±)xÅ?ïwåI¥7ˆ?‹£²h€C…?'VËY?‹£²h€Cˆ?ïÌòjÔö?rJ6¶JÃ?y†Êý•…†?rJ6¶JÃ4FGL J0203.6+7233¿ìÈ@"K¼ž@$ä$=Ìê)À9ÛtÄÍúÊÀ;Ü|©žÊ[@iŠ·( ³@@Tƒæ?½Û"zÿ$¹?¬`áZàK?ðô:æ…Û@0aV݁?íh"ÿ‰;¿ØŒö=^…F¿ã¸j¤ ¿ã¼]ž–®ƒ¿á…òB}(¿èRçcQ0AGNbll3FGL J0204.0+7234S5 0159+723?ïí§'	É?\Ô0
öpÈ?bXô}ö6B?\Ô0
öp¿?ïøÊiE=€?j´²ò?LÖZë
ã?j´²î?ïÁ"6æD?8ß??=óäŒÞ¬?8ßB?ïàK/ˆ?[ÓY¯B6?o´Ðw€ðú?[ÓY¯B>4FGL J0203.7+3042¿êòPWWEÀ=£gŽÀ8—'¡}"À;°-,ˆõ@z<c3@ )»»,'?£N O´Q?¹9@}ôwŒ@¹Wɱ@š³ÿʥ¹ãf_¿Ý¶µÅIK¿ã½ÊÁ.Þæ¿ââ!LÖÈ¿éy"ù÷¨¿è²#3
ïGAGNbll3FGL J0203.6+3043NVSS J020344+304238?ïù.©…L1?K‡‡*5wž?KEYêÏ;Õ?K‡‡*5w†?ïúBÂÙ±Û?]î)íà†•?Fôô™8'Æ?]î)íà†¢?ïƒ&'A?Ç`YA?6_o½à¢?Ç`YA?ïÿG1 ¥^?
›nÖHp?ËëTc'?
›nÖGg4FGL J0204.0-3334?â-}5CZNÀREQ.ƼèÀ;1ºÌð;À<Ïïå։@ ŽÙw*.?û­ L;Aõ?Ó5šìð{?Á61u?ðßn	È֞@Œ_Ó¥."?ïK°¢ÊšÃ¿é÷3þŠ4!¿×c.qÊH¿Öž*¢ëÒÌ¿à$>adŸ¿èý?[_¢AGNbll1RXS J020413.6-333345?ïÿ<­Ñå?lE4q?jEÃFç?lE4*?ïýÔºØUà?Ké+Í£þ?1Z)=Pû?Ké+Í£ß?ïñ,uHW?h˜³Å¶?]§ÏoQd?h˜³Å½?ï÷ô'áoç?@%'Ýeh?PÜ= 2?@%'Ýe_4FGL J0204.1-2919?Öð[ä®1nÀRuæFñVÀ;«*ÏÀÀ<÷P²ŸúÝ@¾žÆ)D?ôÎ3Ÿi½3?âUÝLvÑ?èõ €"Ž@V–8@[ul=ÀÖ¿ÒÞÎWˆ?åõ•äsx¿B­­ê‰v¿Ô1‰$i¢¿ç©$@üõ_¿ïü5ĊßAGNbcuPMN J0204-2923?ïÆÕõ¬-?}8!'œ¿?|•)é~ô?}8!'œ¿?ïñך,'?&;ÛÁ?\PËï¦û'?&;ÛÁ?ïõŸ]ƒÈ?"ÖÚws…‰?œLO†á?"ÖÚws…‹?﫝aú`?y˜ù—üY?…§œg´?y˜ù—üY4FGL J0204.3-3140?æIfÑGõ'ÀRa	éÍ³À;nÈÏJ«À<á4s¥J@&ky˞@d‰Ø[?ÈÐæ¿'æÜjl?ÊîVŠPPz@˽€~•‡¿èòÁS¿ØÔ¹*X™¿å!s¸^€¿¿ä´_î}!¿Îüâ~ºÆ¿å2R˜SH|AGNbcuMRSS 414-035156?ïùøž<Àˆ?B6.͍wð?H‡ýâT?B6.͍wÓ?ïû³¬xè?Y3þ¥›?A1NàYT?Y3þ¥?ïán›³Rœ?pa÷X§Û}?n'dL­b^?pa÷X§Û~?ïü˜
ä/Ž?/ \ØAæ?;?¨Þƒ"ð?/ \ØAæ4FGL J0204.3+2417?à{Y!¥øÀAÔdE#öÀ;8é
55À<¦²ò03¤@ ãóÏ/?ù)p;Ò>&?×µZÀ?ö?Ô
ª]·U?ÿ"!bPW@®A·/£?ïÎ3i¹×þ¿ÒÙxÛ^¿æ†00Is翶Ҫ¡¬¿Ñ¢#ᆘ5¿ïÿ® A§AGNbll3FGL J0204.2+2420B2 0201+24?ïÿ'†©#ù?ÔbS`±?*ۀ¾m?ÔbS_À?ïýИ¡–?Híf%ã?1:óN`?Híf%ã+?ïΞZgÚ\?yAö³¹?x°ÒÌÒ0?yAö³¹"?ïö.U†¶­?F£$Öñ?S£Tò'¨˜?F£$Öý4FGL J0204.8+1513¿î¯ºç½AÀFŸÂ¨†œÀ9Q/¯ðóôÀ<0rÅð9¹@Œe¨%x‹@ª?Ú
£?­ÚÉ呿±?µ=+Y m@ä¢üïªG@ûû˒æ?~Ãvˆr€¿ä"¢A]îH¿ã(Ÿ[zz¿är_îÓ¿êl5恿ïüÑaÜéÐAGNbcu3FGL J0205.0+15104C +15.05?ïüª·Kp?5bœbá4h?;ªE¤'S?5bœbá4j?ïý‡–`éV?M
Åm¤?3ÃLøµBý?M
Åm²?ï~pWí
?‹Çò«½ñ?=1õ^×?‹Çò«½ø?ïûáDà \?24Q_œeJ?@zì}~"»?24Q_œe†4FGL J0205.0-1700¿éêww›BÀQŒí"1{À8ôh§‰FeÀ<DÕòæ<@Ò}'Þ[@ƒ&ùz«?¨x'¼›?´ç<t$•@XxœÉÏÂ@Ôo{bø¿×¬| 9›Ø¿ä¸MžïCð¿èpžmhä¿éŠÃæ¿ïýò߆õ¿ì"ñÉÜW"AGNfsrq3FGL J0205.2-1700PKS 0202-17?ïÿ€/‡;?#ø‰+—?ô1;Óà?#ø‰+—·?ïüÌ4bÃn?Tš0TY•é?9ž\é䐊?Tš0TY•ç?ï³À?/M{?~£¬ˆ.?ƒð4,¡|?~£¬ˆ.?ïþ¨{žÁ? ^kë·n?%xF÷™? ^kë·È4FGL J0205.2+3212¿çÍûd2À<†Â&€À9#T˜Þ‰À<
qÉp÷º@\b}x¦°@kÛñ,þ?«°
ÏK'?²)­ß‡ö•@S¤!²Ø/@<¥Á›p¿ÊuIRk¿åò•ž¸<r¿èTS¿DÎç¿èQ°''¾¿ì1Û¿ÙÊ6¿ácA&
AGNfsrq3FGL J0204.8+3212B2 0202+31?ïþ½M_¤+?W›ír5?$+*½Eï?W›ír9?ïüΌs5Ý?Tì§KÜ"?9‹œfQ&)?Tì§KÜ!?ïÑCS³ç?s/[«d?wx^V&o?s/[«d?ïÿUêˆâ¼?­kCz;ÿ?B®ã¨l]?­kCz;4FGL J0206.0-0958¿êzáV1r)ÀP[2 f<uÀ;ˆv{‡_ÛÀ<ÊXÓÖ¬@!Tÿ™Ó¦0?üámÙ!næ?Ðrñd0×
?•ñ{ؾr—?Çn,ÙQëZ@%v\'É¿áî=•ŒÄŸ¿ìäÚEÀ¿Û̘ÊfÀÿ¿¸4ûï¯P¿ãŒÛE5"7¿à!4-.6tAGNfsrq2MASS J02061590-0957174?ïÿ¡:QbÆ?;|ßÿÖÓ?±k§NhA?;|ßÿÖ¦?ïþ§çCýX?D
ƒìȸ?%‹À*ˆV?D
ƒìȳ?ïú¡^œê?UÓ<°û©<?G…z…Œ\?UÓ<°û©8?ïþÈ9QLè?aîµ2?#|jë1{ý?aîµð4FGL J0206.4-1151?îiàSfÚòÀP­[[ÕÀ8üQo^]À<(.Ï÷#¸@mO–U¨@TdÏ?¥
¸À¦N?¦'ÎI#µg?ýUúX R†@P+ÁÏâ¿Ò×Gd˜…ó¿ãlh'î¿åÞûmÊö¿ãPPzkÖé¿é={Uá³å¿ïÿ3òuÓÂAGNfsrq3FGL J0206.4-1150PMN J0206-1150?ïþ5wGý?@
C#‹?,®è‹€,n?@
C#‹?ïþÍ¡o«?:KB?¶|þ?#%éN×Ó?:KB?¶|å?ïÖ¶m:ç?uÉl¯ µ?t¤ôÉb?uÉl¯ °?ïÿ"<áj?Š$GX'?·pÇ¥€§?Š$GY©4FGL J0206.8-5744¿ÖOF¥±Ï½ÀLP64êÀ:ÌÁTɅðÀ<ÅZã{dû@·´Œº?ülA÷ò…?Í7xý—ÅÚ?ÆæÇ	i`A?úÀÇ¯;@ÿ¥' T?ïÿüÚ±'Þ¿êM"M1â¿ÖKž¤pb>¿Û¥i±t'¿àé"89,q¿ê"]u&ÊAGNbcuSUMSS J020640-574948?ïÿoÝJè?
ç3Í-?V¼BÈÞ?
ç3ͺ?ïþ$"?DåÊId?.í¾÷¾œ&?DåÊI[?ïسée7n?zŸ2âÜ5?s¦MdH»?zŸ2âÜ<?ïô¤Pkg?DQ^À»1?V·_)5›?DQ^À»(4FGL J0207.4-3855¿ïê†;ˆiÀQòº`À: r̦6`À<´zˆ\Zt@5ôå?_@Œ|½ÀÀO?¼J^¼?¾g:vÉ`?ôšøÄ¢[à?üòUû_1i¿äÐG«<#¿ÛnÂÊ £¿åÇ]Œ£¿ëÒ ;I?fßހ(A¿ïÿõ¹U ÄAGNbcu3FGL J0207.9-3846PKS 0205-391?ïñÄÌKò?`ÞN˜Nà_?]övgh ?`ÞN˜Nàd?ïìWâ"q§?y¨
¦d?c¨ݎX?y¨
¦d"?ï
ˋ%Äû?"œÞ±-?žFŽ›G`z?"œÞ±/?ï×x‹W³è?júÚðJT?tCºT&]?júÚðJ^4FGL J0207.5-1049¿ºˆˆsS£ÀPr½f'|À;^ìz>À<—6>@!¯vz° @êE%£þw?ɲN¨Ú¿ƒdZ¦gr?¼ 
|xˆ@ã9ÇÝû¿å™‹¢
+}?îñŸoÇc¿é‰Êï|û¿íJU^×&?ã_Nyà–®¿ïúÛ2ÁlAGNbcuPMN J0207-1047?ïõÅ(|t?\fðËhÖ ?Tu¯Ï?\fðËhÖµ?ïþhÚµê?CÌN$"h?)r^$¡b~?CÌN$"j?ïà§5??ŠúRrэþ?ëX?ŠúRrэý?ïÿ8vn¹?[š&n6?ñ20õ2?[š&mï4FGL J0207.5-2402?î®îó"ÀR$œM©?À:F´ -œñÀ<•S–€	¦@̓P:@FúZ¤'D?·¦53h2?Dd!×Z?ã€e`WÆ@*'Bðë?ìpÐL´
¹¿ÞJp¼€¤U¿âŒ
¿Ü$¿æC$Aþ¨¿Ô³œzª¿ðAGNbcuNVSS J020733-240202?ïþ Iݞ'?!â¯?`*r?%ûb&ô?!â¯?`*?ïþ–Çèе?@1å%p^Å?&"rô¿û?@1å%p^â?ï܅'ɺæ?tmýâü%o?q½6›"Œ{?tmýâü%q?ïÿ]½9Ú?3Œü?]Xħ?3Œý4FGL J0207.9+2203?ã²*
‡€ÀB¹v_Ø­¬À:ýîðäJÀ<‰iêe;@AhÃbì@5ëÄߘ?ÊθŠJœ0?ÊRøJ~ÿ:@
Vz`o?ÿ2]šåÉô?ÔÚ³àl¼Â¿ÔÜõ8ü¡¿Ëe*§µ¿étËNG‹°¿ÌiýIÂ@Ø¿ïÿ€éŸkkAGNbcuNVSS J020801+220241?ïuÔŒ®?†[g$ßV©?ˆ¢Šû\Ô§?†[g$ßV©?ïâ `È1?ƒ£¹{}?mßäŸ7Ïm?ƒ£¹{}?î9 o4á? ý'½å/?¬mù±çã? ý'½å/?ï"¾øY@?Š=Q˜Ln—?œ¯h ô×ó?Š=Q˜Ln–4FGL J0207.9+0953?Ê!ÚóU
2ÀHL	¢@1HÀ;U&£øÀ<a"ÌÐþ‹@ƒÌ_"?ü³^f½¤?Ü~9¡ŒW<?ïû¤$èî@›Ç;"T@¢°çiR?ÒËA&»×¿Ó"2ëƍ¿Ø{{vmð¿è  ‰wãf¿é¸âό¿ïüÒÿ@èSAGNbcuGALEXASC J020754.55+095014.0?îѤŠ3ʆ?¢4ŠuÏÆ?¢å·\ÃW°?¢4ŠuÏÆ?îé8IõPy?µ,÷ ‰WV?¡l{`ªøo?µ,÷ ‰WV?ë^6çnœG?¨Äãtl2|?‡$bEŽá?¨Äãtl2|?묬¯>d?²XNÕ4j?ÅMMCo?²XNÕ4k4FGL J0208.3-6838¿é¯@4f‰ÀGyÂôÀ:oî'B³À<£ˆÁÛC@F¶š[`y@uIÞpc??¶ØrGp,¿£=Fÿ».?îó^ÂC|@¼3Æ«öh?ï0hå¿¿æNèÑQ­¿ç|>¿ÙI]¿äÁgÿBÀÅ¿Í
­B˜ÖÑ¿èÿ[_¢'AGNbll3FGL J0208.0-6838PKS 0206-688?ïü^6•–ž?4ÇU]æ.^?=KSKo?4ÇU]æ.:?ïþ-£EÏ?GL–eÍ:?-%Ë£¡I?GL–eÍH?ïñ*ûØQ!?gOåÆjÛb?]ªO]½Ç?gOåÆjÛj?ïú
wvy?9«XY~¥Æ?GÖ"&ù?9«XY~¥­4FGL J0208.5-0046¿á¦oÎô'åÀLæ…3±tÀ:™ôàèÄÀ<Ã¥Üû@œ=n€@§¬Y¾O?ÀD
Ý)¿~ÀŽ–—m?Á™ÁÕ?þ¶E|â¿ãÑx=Sr™¿âDr@bï¿ål"ABÀ¿Ú5…=A)¿ì4"|+ʉ¿ïÿý±q&´AGNbllPKS 0205-010?ïæsýM¹+?dÅy¾´Ç?iŒ²FՖ?dÅy¾´Ç?ïæ
¸Ïø?"=1€§ô?iõG0ì¥?"=1€§ô!?ï‰F$8?ŠCõEK?®[à6ñ­?ŠCõEN?ïÏ3–΢î?hÔc7#a\?xf4˜®‰Œ?hÔc7#aX4FGL J0208.6+3523¿ÙÙ©΁À8ÞT´:çÀ:¢zˆ\ZtÀ<|î¡2ë@ ¬í†««??üä17°pv?Ãìmçd'È?·ÛCÝûH`?önõ›øïk@7Áe¤8?ÑÏ3"f×z¿ßSȟ@¢‡¿ÞµÿÆÜ¿Ñ	žD#E¿áÎW±—½!¿Øµ€ëLê"AGNbll3FGL J0208.6+3522MS 0205.7+3509?ïû›€ÐÒ?<KfhðÓ?C‰'ü¼¶Ñ?<Kfhð¹?ïý|Vp¤?Pº½Ï$
?7"Lzàb?Pº½Ï$?ïò¡d@©ü?fó¯Sz?Z½7~¬?fó¯Sz?ïÆKƒÝ?c\……LÆ¢?|øøÚ>ë?c\……LÆ 4FGL J0209.3+4449?ß;8ö«À/À¯¸kÀ:r™A…ŽÀ<|á®ai@ fŽ›ê'?ü€0ŒÅÛ?Äò™åﳂ?»!²,b‰?önøÜP@@[Èµ¿ÈE»K¿ç³l|*¿Òf'åK†¿ß§üaåοà••_x6¿Ñ,Ó}kÃAGNbll3FGL J0209.5+44491RXS J020917.6+444951?ïÿ9®z>?¢WL¹»Õ?Ê0¸=ކ?¢WL¹»ñ?ïþ%ü÷'¬?LlW€ïã?- 0…M²?LlW€ïå?ïùCǷď?^'ÓøÁ?Jðá íƟ?^'ÓøÎ?ïó°Œ(F?CâßÍã$?Xžç¯Ïu$?CâßÍã"4FGL J0209.3-5228¿Ó¾ˆƒ±ÔuÀNb$‡wÀ8—ú…l»ëÀ;º•µßJ~@cŽy*
p?üêzAå}ž?¢î½¾h?žFøaûó?øù5
£Çñ@ Àžìå?Þ5ëŸJÞv¿ÐOõ
ÙwÖ¿âi%]‡›¿Ó­vÛ©‰|¿àKm̌¿ÖG EDØ¢AGNbll3FGL J0209.4-5229PMN J0209-5229?ïýìYl—?-wÆ3U˜X?07<›BX?-wÆ3U˜i?ïþ-ìêá"?A‹œiÞŠ?-!1Qç½	?A‹œiÞŒ?ïä«;—t
?u[̃9-?kTÄh‹õ¿?u[̃95?ïýÝ>{ÙO?&q¹Í"v?1!5–é?&q¹Í"ã4FGL J0209.9+7229¿ïü-\Fñ¡@%àŠï³À:ZÄq´xÀ;ïËWÇ@[ZÈ£r`@›ß>¿Xp?ÀºAYç|ü?Ñr»´K¢@í¬«ÅH@;OŒZA¿åå¥ `r±¿Ý§4ø/Q&¿à½¥6Ü¿àŠ#opÑ#¿étNáºo¨¿ïÿ¤àõx¾AGNbllS5 0205+722?î'>—.7?£©´ËÀ;?§Þ,£?£©´ËÀ;?ïõ·HÔó?gêâz!ž?U֑nV1?gêâz!¢?ç{ŠmœK?°îAPï?Ñ	Þë$Çi?°îAPï?ï÷®‹ÝåÇ?C:Âeó,?P¢èD4qÉ?C:Âeó 4FGL J0210.1+2518?ïþZ'6ÀAWÿ›V2À:ã쮤"À<_ˆü"d@ 6Ä÷@hÑ?ýéXÎG ?Èív{†'?ÂèSX?úþ³†ªª@ †ó¤§ë¿ïŸr÷na?ïD1Rˆc¿½"ëYÕ´R¿Ú`χã¿Þ»S'Å@ç¿éþý×0ÓÝAGNbcuGB6 J0210+2517?ïû—l¢»ù?A{¹>ó²?A¢Mu½?A{¹>ó¨?ïôⒶÍ?tÐ:û«Ú?Wü:ڒeä?tÐ:û«Ø?ïÈ›Œ'?z2=/,Ï°?{ø²t9ì´?z2=/,Ï¥?ï":àÚ?{Ô:TÁ?ŽñGÉ~|[?{Ô:T¿4FGL J0210.5-1445?æ<CŠSç/ÀPõ!…Æ~À;0|ý À<®6Ýß@Š
D·)@í¤Ûìû@?ÉøǼ톬?–C<j¿fˆ?Ê:ÜúA@S>"u¿ç`
¹(*¿åõ–àVÂZ¿äÅêà´
^¿ç²PIÄo0¿ÂªÍ‰
UC¿ïü¨AÓ	'AGNbcuPKS 0207-149?ïûák/ˆ?<jö!
ÜÈ?@zS·AßØ?<jö!
ÜÊ?ïýÌx\^Û?SpÔ9Eå?1œ=	 P?SpÔ9Eå?ïÈ1ÅÙ6?xim÷É,Õ?{ç@dØ?xim÷É,Å?ïþõˆÔ?%Ÿß{
ã?.ð®grÂ=?%Ÿß{
ã%4FGL J0210.7-5101?îô8»ÐÀNã
ⴖÀ7Žî&¹¨-À;"Ë7¡W@ª¢%.b¿@é¾?kOÚ?"yy»n?µÒÿTÿ6@!þÃüC²Ý@7hÿóÀ­¿Ï'X&`¿áûúëÄ	¿ä¶U⊤3¿å桇N¾¿êÕ#³co;¿ïÿÈ¢› ÛAGNFSRQ3FGL J0210.7-5101PKS 0208-512?ïõÜàÀìþ?M	yɨ0?TF>~&u?M	yɨ/õ?ïç>™C?{òÑ'^Á?hïÁfî¼À?{òÑ'^Á?ïqÌÒxe–?Ž_Á†G4?'Æe°óMW?Ž_Á†G9?ïõSˆÂ¿?Lz|Ž ¶m?UóXîz€î?Lz|Ž ¶y4FGL J0211.1-0646?ïŽrü[ø'ÀO.œË}AÀ:­ß1S_À<œÂ?«º@bWšÆ•P@ˁ½?ÁÛק·?úàe8?ÝÃn_E°@Õÿ¾^Ë¿â<Þ1;¿ç窟ѿÐ?Þ½:3¿áólß&k¥¿â;‡•‹¿ßPå€wߋAGNbll3FGL J0211.2-0649NVSS J021109-064551?ïþ§Óyµ?"æcãvuæ?%'Èd¿…?"æcãvv
?ïþÄ
9lž?D¤&ð¢b?#¿,i6U?D¤&ð¢]?ïõʹŽÖ¤?eƒ°dÔò?TjŒâR¸Ë?eƒ°dÔò?ïýNÆNh!?&<0Eqo¸?5‰ÍŒ¾÷È?&<0Eqoã4FGL J0211.2+1051¿Ë¬Læ«ÀG¯Š	ÞÀ7³´&ÚÀ;FÀh Ó@ìœf}t@hG,{Ä?—œM9Tñ…?ªÑÆþùè@¾×@Än@çuK[ž?Á]GXÚ¿Ý×Êâfçì¿âÿp"§Êµ¿àúLÍ8,—¿äÀD=Njſä.¢<ÖAGNBLL3FGL J0211.2+1051MG1 J021114+1051?ïý2Ñ•
?.ù-—¼è?6iwCW±K?.ù-—½9?ïó¶8Qá?r a"a÷\?X"ù\@Ã?r a"a÷]?ïÜ×`{ÚD?xD:bÙa¸?q"OÂÝ??xD:bÙa½?ïû2?fªl?3F'#¯öa?C7eVTv?3F'#¯ö…4FGL J0212.2-2559?î‡cÑЬ4ÀQú¢‡~äâÀ:þŒjÜí¬À<·†«€L@´Û%«
Z?ý#·ÊÝ"?ÉÈ#š¹Õ#?½.ëÐÉÃ?òðñõ{AÀ@¤ýÒ(V`¿Á‡
`V,¿êHº–i?­¦ŠÃ½Úl¿ã¤ÁëÈ:—¿ÞáAäP÷ê¿ÖޏØO·ÎAGNbcuPMN J0212-2558?ïþ!lõ¬
?0¯œ?-é0¥?;Ü?0¯œ·?ïü¡íbä:?R}€=ï?:ð"èÞ'?R}€=ò?ïíC
ßÙ?lO?3±O?b¼õ~ %Á?lO?3±A?ïõé¶^?E–ì쇷o?T,"ÕÕDp?E–ì쇷"4FGL J0212.2-0219?âGÛ`)ØÀMDÁ~ºñÀ:åG5H·)À<£zm"h@:iàCw#@ƒýP"WC?Á·ýO0À¿š6°¸'xÛ?ÕÚSÑä@…ѳ'gq?ïçu$oK¿â#Ê|"¿ãÍug‹*¿åPâÁ*Ø¿Ü•ƒŸÝ*"¿×¶ %#ûÞAGNbcuRX J0212.3-0222?ïþkúY&S?!ùÀȳ?)@ZmšÅJ?!ùÀÈ{?ïþÆ|è
æ?B±òݸç?#˜1!«s?B±òݸç'?ïòQ#8µ?fe;Šùƒ?[]¹Žz™??fe;Šù?ïüŽßçR	?*ى?×?;‰Åo¹w?*ى?ú4FGL J0212.4-3502¿ê4xm"Z
ÀQ¾¹¡vÝ­À:Wõ ¨ìôÀ<«©f–7@j¶JU @3T¦J'?¹ÒœÅsE?ƒA©ÝMg?ÉÖ§.ë{@ƒC¹=N?ÑEœš*
¿æ·½ ‡_¿Ù`ÈWG¿ÞAàËy¿å³2'#ƒ"¿Ê	 :2*õAGNbll3FGL J0212.8-3504RBS 0292?ïû-±7K?9›©zNÊ?CKí;"Ӊ?9›©zN
?ïý÷ ՛?Kª5y?0FÿQS'ï?Kª5y?ïó~kÙy?kŒ*§¬9&?Y(Mû&?kŒ*§¬9?ïû3)ü°?3È~L/u?C3X
@?3È~L/4FGL J0212.8-2721?—ež·šå·ÀQû†ìë¯À:Ìb¯!ÁÀ<·îŠŒ¶\@2œ"uÃQ@CTc.£?Áö
HX^f?¨Dͺ]‰s?ä鋧i@#f•á(N?ïµÖ±R¿×s×}ªÐ¤¿ãZŸ2ਿé·?Ò}涿Ì=$ä
d¿ïÿÿÊPËAGNbcu3FGL J0213.1-2720PMN J0212-2719?ïù4t"Î?MÜ;jmv7?K/–-°ÇÕ?MÜ;jmv'?ïüxٝÌ?VaX›fnN?<93Ÿõh?VaX›fnO?ï'M{–l
?†Ó192 ˜?‹l¡dü‹?†Ó192 œ?ï÷3"VV?CmqŠM?Qó˜ÙSV²?CmqŠF4FGL J0212.9+2244¿Öˆžl±&ÀB/ü~k?êÀ9ÐK¨ñÀ<<µ…ˆj@ð2¸9?ÿäçUO?µó8ò9î¹?¾·]¤ËÑÐ@
/»¯n@õÆžh5¿îÑҀ@M?ïæ#J‡ã¿àËÂFa
¿à¥0 Y;Û¿ä<zo1ç¿ä÷ƒŸ‡DWAGNbll3FGL J0213.0+2245MG3 J021252+2246?ïúVÎÕ?J½Ùï¾?GƤÇĦ–?J½Ùï¾?ïö鏍fÀ?y/ç뚉?R,àå2»?y/ç뚉?ïÊüÞñÜx?zßHBꙧ?z‡Ą?zßHBꙧ?ïÐ(«šùü?h14$ÿâ?wëª2ƒA?h14$ÿë4FGL J0213.8-6949¿ç"±/f¹ÀFÔ×ðí=†À;!ö'õ;À<Àµ™ª`'@"5Wâ¿þ2?øáv<?A?ɂý5uWÆ?¶.Ý8)è?î'gbÂ*@ÞÇÌÿ¿ï³ «Ü'=?ïõf4€¿áÁçâÒɿ؀Q~Í»_?€>—•]tпârá锄AGNbcu2MASS J02135882-6951360?ïÿ©	'Î?* d?½½ßL9B?* ²?ïþlž^V?CtkãßÑ"?)6ª¢§?CtkãßÑ(?ïõ+£Çî¸?Y+­Jy?U¨¸p"Ò?Y+­J¢?ïý(ª7OF?0ú;ƒKMŽ?6º®E…Ç5?0ú;ƒKM¸4FGL J0214.1-4733?ïÇrø׳}ÀOù
¿cíÀ;€£n.²À<ê»ð¶ù@ qâ;žè?ü#æt=¿~?ÝΟ C×Æ?·_Kêå?Þ±]û³À@ßyw»#¿ä¾¡@W%¿ËâäfF…ö¿ã[ºÜ	€²¿ÍÍâK ¿ÛV,\\׿ïó±"L["AGNbcu2MASS J02140989-4732357?ïÿyÒHô?—å÷!?ÌE¶áŠ£?—å÷ m?ïþ&!rêJ?FH†š¼c&?-èÑ[sØ?FH†š¼c/?ïÅ~H—L?…+UáÀÿa?}@Û´ZÁ?…+UáÀÿd?ïüiVñ?0ç÷4â?<µHs÷³®?0ç÷4áö4FGL J0214.2-7025¿ÜÝ&aê¸wÀF[ÕìlÀ:)?—Å"À<vׇ:òD@Å´Júz@Ñí@	ÛK?¹g'Ñ_Ú?°¤žìzù?ðB'!¬øò@?q¯ðž¿Ü€'q^çí¿ç@D"­Ç¿è'&ëý¼¿èéé¾4ú¿íA8D,¿œµÐ±Þ´×AGNbcuPMN J0214-7027?ïæitôx?hOËAœÜ?i–‹ý‡—?hOËAœØ?·iîE?"|GÑöŒ°?€R%"n˜?"|GÑöŒ°?ï%»Yšgb?'¥Aʪ?›H"̳Å?'¥Aʪ?ï•%@eÉè?yèpk¼|ø?Š¶¯æ†6?yèpk¼|ó4FGL J0214.3+5145¿é0€n÷À"s2&ÄÀ9÷kÅJøLÀ<C:8
2‰@ ›ú©ÿÃD@ñ›¹.Š?®CµâO•ê¿´'HnXÎ"@7E«I@ÑZÚôã?ïã)›üå¿æ™Sù|X¿ã«xßdÔì¿Ô±qÝ=r¿âkí>\\!¿ÏÑß[DÊAGNbll3FGL J0214.4+5143TXS 0210+515?ïöŒ·ù?PŽ>MlŽ¼?RçÍü?PŽ>MlŽº?略I²¼'?­R!9 ²?†'m"Pۅ?­R!9 ²?ïÊH"Âú?€=u=´?zÛîòžƒ?€=u=´?îð'¿…r?ƒÞšÜ(õª? ÷&Ô¨ñ?ƒÞšÜ(õ«4FGL J0214.4-5822?à眄ž0ÍÀKÇߏG0@À;}ÂO›HÆÀ<òÿ4(%¹@\E*¯}?þû˜\'·Ö?ÓG÷›,–·?Ԙ\bq?ýëWfï"b@
ôù
†¿ïQ¶
éh?ïÞ'bEo¿Ü—û3èe¿âÎcûR¿æU.enâ¿ïÿü¥¬¨AGNbcu3FGL J0214.7-5823PMN J0214-5822?ïþsR²'?)únÁ–bb?(Ê×Öõ?)únÁ–bL?ïýI†T'?RÝÌZÛ%?5³Ï}[yv?RÝÌZÛ?ïI¦þ`ŒÎ?'J°_*?–Ë 3îfB?'J°_)?ï÷ÿg9Ý?DE"§«ñ•?Qè1ŒD©?DE"§«ñ4FGL J0214.6-4333?×xÕñ•yGÀP Ž4À;ïiÃèø|À<ü]¿Î·‰@"Ù¾9a«?÷ Â'Æï=?ÚrÁ`'?²Ì)cы£?×"ªú¿ú+?üøÃñ11?ï¨HSUèj?ØãŸAyG¿êcnÏÁsÓ¿ÉÕ	‡=K¿Ðu¬¿ç<¿Ç""7ª¼,AGNbcu1RXS J021439.0-433319?ïþˆ¢éN¤?-ì»ÖÈ?'uÑk¬¸?-ì»ÖÈ5?ïúO8TªÁ?eU8rïm!?FíTþô?eU8rïm!?ïՈù_nÜ?y\¡šŠÿ?u;ƒPH'Ð?y\¡š‹?ïñ<[ª?Sø"MÙ§¿?]‡×Iàªi?Sø"MÙ§¶4FGL J0214.8-6150¿áj`ûM´ÃÀJN(ܘëÀ;6¬7+xÀ<ÄR)˜¾@Pþ39é@ˆwîN&Õ?Ð|³úîÉ!?Ð>͛(åÒ?öýã¼Ó[?î—õøó¤Û?ìŸÝJÉQî¿Ìôœ_ÄW¿å`¿'țæ¿ç[`m~¿ïÿ Êƒ+?ïôìp×±AGNbcuPKS 0212-620?ﺝÓ1³Ù?Šz­‡€b?X‹3"	­?Šz­‡€c?ìo×Üa`Ê?Ékg$Rõ?¼Aôù³?Ékg$Rõ?ì+Ä«½?¥ŠV‰wK¾?¾¡ßR§?¥ŠV‰wK»?ç@‰DiXÓ?¹hIïŠî??Ñ~íw-NZ?¹hIïŠî?4FGL J0214.9-3722¿ï@lÃ↧ÀQip£×
=À:Ç	á*QãÀ<¡ jْ®@»ˆçÕ@S3¹jð9?ÇàáÂ'W]?±>lwL"?äq|^ö/@¹U¹ÅÞò¿°ˆUà˜lÚ¿èæÙóü¼¿èyÞp¹&¿ïÿ·äkO?ïîÑk%¿ïáûÓJ•PAGNbcuPMN J0214-3729?ïÿ—œÔ19?õ'qÙî?
Êó±—y?õ'qÚ®?ïýËYãe?Q'Ó~¹a?1¥7¸äÐÐ?Q'Ó~¹a?ï©ä2¦×´?…çë2\?…†óVJò?…çë2\?ïÿyòï{^?Ä°²k:@?Á¢"O?Ä°²k9Æ4FGL J0215.3+7555¿çå=ð{@+ÈÂ?«ºÀ;)A® 9À<˜?gôÛà@"cÑeõ?û!DˆÆ¿?ËlØÆU9m?ÀDc²,
?õ#|ÜÊpÒ@'ÇœŒ=;¿ïÿîͨ"ß¿ïüúAzÓ?ïÿÿ^ðP`?y7»ûe³Û¿å&Õ!/$±¿k7¯çUAGNbcuWN B0210.3+7540?ïþlÄn#?#¾O!,üÜ?)3¹ýÔ*?#¾O!,üÈ?ïú'ûO%?e7'ñq]?G`Óp‰?e7'ñq]š?ïð³JF7?cʾ_î%Ê?^™ksó"ã?cʾ_î%å?ïÞy94‡,?gˆÑ"ñ‡›?pÃce¼i'?gˆÑ"ñ‡"4FGL J0215.9+0300¿ïäeA1ÀJÏO'õfÀ:Ÿµ<OÀ<wRœ…e@›	³Ýè~?üðÏÆ|P³?ÍJ‹¼[?ÄØOø:ä­?ø¨Øœ
è @)_SL®.?ïþdŸfã¿èK7 }£ð¿Þߤ¬ó¿Ò¤^Ƃ;¿ævîÿ|¢h¿ç,Sæ1!áAGNbcu3FGL J0216.0+0300PMN J0215+0300?ïÿSuzY'?84ºÌØ?'P´ÏÏ^?84ºÌ±?ïýGc¹œy?Rzi¿ÛFU?5Äâ36'?Rzi¿ÛFW?ïÜ(ÈF×­?w¬¡âL6F?që›Ü")?w¬¡âL6G?ïë×Z'ҝ?QãŒÆ*o?d(¥}-cb?QãŒÆ*f4FGL J0216.5+2313¿ìXüdþÜÀAÍ®_ú;›À:'{&ÁÀ<deÀN9I@ º¦'Ço?û)—Ãք?ōK±?Ç@÷Ií@Z	`ÑÑï@=*WíR¿·²Ãa>3¿ê‡/3Ê1è¿Øì]Ù¤÷¿ÒHj|öu¾¿à¹Ã_eÁ¿âsè/(âwAGNbllRBS 0298?ïФ+v¿?r}ç9íÊ?w­êD €—?r}ç9íÇ?ïôb"Ü?€ïõÄ
À?W:×ÕâCæ?€ïõÄ
À?ïgí†êh`?KÈZá?"O"²ô$?KÈZâ?ï¢ZÖoQ™?tGK´eõ?‡iJd+™€?tGK´eõŽ4FGL J0216.6-1015?à1ˆýo0ÀO䦰)(À9¯'OH<°À<Sû!sî@´¹¯ä‰­@ÑÿÁìžú?²"¡9öñ¹?¶"^—&@rá& %9@/«$ÜX[?ïØ~>õ3¿á[CÝOÒ¿â(ey×\s¿à峃O«9¿æN'b™R¿êdüAGNbcu3FGL J0216.6-1019PMN J0216-1017?ïþ¿ø"¼$?4€3zÀÌ?$vÄ=¾1?4€3zÀe?ïþP‡uS(?CH'9ÄÔ?*÷ˆªÍ">?CH'9ļ?ïÝÁ-h4P?s¥KÉ·h?qiKåØe?s¥KÉ·d?ïþ?L‹Ï«?&/îb@?L‹Ïy4FGL J0216.8-6635?УC‹@ÎÀH2â\
WÀ9ßæÆsxÀ<A,…šT@ˆ€UÐÁú?üšÊ¡yaì?µ³›ÎR2þ?ˆÇ#ël @1'o°'@Oìú"±'?ìÕsd{ª›?Ä;å'Ûg¿Ýá\†Ô¿Üi.âìsÜ¿âžaÔU¿çž|øy#AGNbll3FGL J0217.0-6635RBS 0300?ïéœÉ€z?eeÍPay"?fc6…€?eeÍPay'?ïëh÷å?•¸ºJ¿Á?dù—ì;?•¸ºJ¿Â?ï&Ť–?—?ïl«EÞ?ž;'_kmg?—?ïl«EÛ?ï¨?¼Ò­P?m‹Ys°»?…ðËT¬<?m‹Ys°º4FGL J0216.8+0510¿²×¼o'	JÀIÕg–ØõÀ:¶ÿݛQ*À<"YÙU@ñiî†0@­õcÄËw?ÂN´XŒ´?W.0ͤÏ]?•ü‹^öä@…>œÈÎ?ïóg ù	l¿æ¦I«D¼È¿èZ9œÙ¿ú¿¸
¤ô–•X¿Ýв_Ž0¿ïþÖ4T›cAGNbcu3FGL J0216.4+0507NVSS J021655+051018?ïû빨\?7ÿJþD?@Q^†[?7ÿJþN?ïýԕ7²?Jbm«ø1?1[VG2is?Jbm«ø ?ïï!=VÙ?bÕÄ3¶¤–?`ÞÂã©&›?bÕÄ3¶¤•?ïøjÈ!/U?<ª-n*ÑP?NTß{BªR?<ª-n*Ñ<4FGL J0217.0-0821¿Ñ‹v-@Œ3ÀO2q`•l
À: ZUÖÀ<t¿û-2h@¨0lYoˆ@+œ›¬™Q?¼ð¢…?À•ÙE¬¯@Lz-È?þ66ò?ïÜ3<mn˜¿ãb€u¿å0éý_;пåv•ˆ'á¿çŽc_öµ©¿ïð"¡!1AGNfsrq3FGL J0217.1-0833PKS 0214-085?ïA‰P:]ò?7Záá}?—ÎÕø´AÙ?7Záá}?î.Š¡Ã[ª?¸V)+Väý?­UãÊEu?¸V)+Väü?íxúúâb_?¥ëÂÓD¶­?´8((ìí?¥ëÂÓD¶­?ë¼z!v"§?¥‰¡ÅCÜ3?Áz%­d?¥‰¡ÅCÜ44FGL J0217.2+0837?â>^c;tÀHQëcÉÀ8­43ä3À;é=~æì@¾»Ú(Ö@ì·M߆ä?¤	±ãÃ?¥]™@áÐ?ÿ¶¢Ù´;Ü@ÈBS6³Æ¿Ò¼ççÛF¿ãeøí½]¿ã»'Ê°h¿âë¹VÎBï¿å҉øÌ¿éJñáeAGNbll3FGL J0217.2+0837ZS 0214+083?ïü–kìá?3S¥=œCÓ?;O, ˜õ3?3S¥=œC¥?ïý?­¬#?J7}Ë°&?6'Ÿ&í	?J7}Ë°&?ïÏçsmU?€àc¬·nØ?xFrÉUô?€àc¬·nÕ?ïø"àêÊ?AÅOÄU(0?Mì|WÄ؄?AÅOÄU(%4FGL J0217.4+7352¿ïÙ֚JŸ@(âCV–æÀ9͌æ,ðÀ;¨Ó5œ™ÿ@—Èe^ÿ@tŸM¡?²ÒRȤÉù?ºÒ	!¼¾7@Ý¥b$¸@
»ž8¥8¿uv×çvà÷¿æïÖòÀ|\¿ëhª¾¯þ‹¿ëÕjËOõ¿ïûâ~å¹-¿íÏîõì€ÇAGNfsrq3FGL J0217.5+7349S5 0212+73?ïú¢e=?K
'-×Ú??Evkó·	?K
'-×Ú-?ï™{pGO?©¸ÅèQ?‰¡;cî,?©¸ÅèQ?ï("«Uqt?'ëîùÃ÷?šíŠ•QÑu?'ëîùÃõ?ï`ÃíI?"A¼©%?"ÿç'VÝA?"A¼©%4FGL J0217.8+0144?×=k†nû·ÀK5 @|ÇÒÀ8DôètÉÀ;¬šˆ¬âL@ÍVnjñë@FÙ='©?X,€«Oé?°X(àôÌñ@Èí_‹Î@ƒxOÇéc¿½ñ¾xÌ¿áU74I³¨¿ã¤ô xÆe¿âŽWF7ò¶¿æ~c³-¿V¿ìì¿0|uAGNfsrq3FGL J0217.8+0143PKS 0215+015?ïþž>K´ò?"úFømí±?&D°ÞÐ?"úFømî?ïù¼…Ýç?aîi'F¦?IÝèˆf¼?aîi'F¢?ïàüwN¦R?u¹4Lä%Ë?oˆ±Y®z?u¹4Lä%Ñ?ïÿ?>=m?‡…Ûä?8P9s?‡…Ú"4FGL J0218.9-2305?ÝàÏC'hÀQt_®¼@ŽÀ:"WÀ±5˜À<žù˜òc@"ÆóÄÞA@˜Ã`<€º?Àb–P9?¦À#Ç‹Ö?å'"^#̹@š?Ĝý¿ÕfÓP0š¿è,ÀÞ'¿è2µ>»§‹¿àÀ;Ÿ=r|¿ïÿþªJl?äcãÏßAGNbcuPMN J0218-2307?ïÿ˜é†f?]I7ò?	Žf–?]I7W?ïþªôx¾?GÓ¼ô²Ô¿?(P¸t"?GÓ¼ô²Ô¿?ïîû= +5?b—'Nö4]?aÂßÔÊ¡?b—'Nö4e?ïÿžEª6â?ÎßÖ?n•rGpm?ÎßÖîŽÒ4FGL J0218.9+3643¿ì7ƒž¥
>À6ê1…ýÀ9œze ì	À;˜	ÿ÷@¥³/³ø@ʅ4-?¹¶ˆèœa?ǤC@Çpl@
f|¼A%@``?°Å¿Àß]ނÐ¿änôËG<¿å=ù*"é9¿çÑ`°D
¿í>"z~K¿ðAGNbcu3FGL J0218.9+3642MG3 J021846+3641?ïéBþbô"?b0eâd¸T?f½kV?b0eâd¸S?ïü»†÷iž?Zp2f.éè?:#ÈD³£?Zp2f.éß?íIjêÙü/?¤Gn8§Ø"?µ´¨©0'?¤Gn8§Ø#?ïó¹TöÃÓ?J‰§ ­n?XVxZ9?J‰§ ­a4FGL J0219.0+2443¿êœ°ÞëÙÀ@ÿÊ}g3ìÀ:T6KìhÀ<]°<sMÕ@ {ÂqÔ¯?þBÙÏÏ?¹jàHª"½?œ}¿ZÑæ?åT*Ã@LÌQ#ß¿ïW‡Üóö?ïÿ˜0ã͚¿äQ™_â隿àcRµ¯z¿ÜJ±ŸIÜÿÁÈpMLAGNbll3FGL J0219.0+244087GB 021610.9+243205?ïþMç€?.!¤ÂæMP?.Ë'ለ?.!¤ÂæMe?ïýlî{Í0?P™¥Éu.?4˜Œ!–?P™¥Éu5?ïéàŽøë?n_hB¶}P?fàq4?n_hB¶}O?ïê'ó›P?X~ºGu¸?eìØd°8?X~ºGu¸#4FGL J0219.1-1724¿ïftùÍÀPã9–ú'èÀ:Œ/•ïÀîÀ<€šl'p‡@74:DI†@ÖßZn
 ?ÀZâ9E›ì¿m;8€Éç?±cDë@ëÔZŠ»¿åPVY¨é¿æ%»`"¾Ž¿ç)%]‡š"¿Øë/þË¿Ôx=({¿ïÿÜßi‡ƒAGNbll2FGL J0219.1-17251RXS J021905.8-172503?ïÿ\g³#?=C>?´s	›Øž?=C>l?ïþ§°®#ä?A#gû*?%"õÁµ6?A#gûP?ïùq'·!'?LP¦¦@ñY?J9µ#yöÊ?LP¦¦@ñ7?ïþ¯[,V?Ì	GôÁ¢?%
Oí:¦?Ì	Gôš4FGL J0219.5+0724?è«Ó_tÎÀH³é ÀièÀ:ôBŒüÀ<cÀ›f"@ YC=A@mY9?È/Á#K^£?'ûôW«7§?ÎõŒI$M@¶ÜuŒI?ï©iñ5aâ¿åÒ%fÁÕù¿è¼Çf[~¬¿Û¸‰ÿr¼`¿ä ~æ¿Ûš©CÛ¡ýAGNbllGB6 J0219+0727?ïþRދ²Ô?#nþX•òÌ?*ÒDÒ»?#nþX•óN?ïþ'æýt¤?G9ŽÕêcQ?-(µ¹&?G9ŽÕêcg?ïø>$çH^?]j?Olbޅž?]t?ïûVV'?3°pƒfe?C²¦§aÎ7?3°pƒfe4FGL J0220.2+3246?æ¸i LèÀ:z|¨"2À:‰m–cÀ<QjúIݚ@òÞÜĽ@^ڀêv?Îj'ÅêÛV?Ô:è‰A@s¹»x³@øE×î¿¿à¶l¾o;ø¿ãt°¨©Ø¿ëMª½Ù>ö¿éx՟eæ¿ïÿå(
eC¿ïÿþÐñAGNfsrqCRATES J022048+324116?ïþ¥JóÑ?)CÄ|Ÿ(·?%«PÎRäÅ?)CÄ|Ÿ(¡?ïë=Š?wÑGz1ݒ?drÂouë#?wÑGz1ݑ?îýþ¸iÍ
?'›U·JΑ?  yc/J?'›U·Jΐ?ï Lu±|ù?v"¡ˆ¢X?‡ìⓠÁÔ?v"¡ˆ¢W4FGL J0220.8-0841?ïà&rËÀNúˆ&ªŽ´À;SôÁœ¬À<´ÚìJ@–@!–L\yþ?÷Π/µÐ?Ôê&yçL«?Óú†c±Ö&?ÿ'~þà¹@W#	ðCÊ¿äúTû½¿ïÿ"Þï?ïá³äžzª?ÒÈÌøk·¿Þ~½_ÇeÛ¿ç:d_¦ßAGNbllRX J0220.8-0842?ïý2Kê¿@?7(l¬¨?6m ªþu?7(l¬¨7?ïýàbbg«?HċIóß?0üìì©)?HċIó·?ïÔáPT¿í?w—f½gÂù?uWÕ 	ï?w—f½gÃ?ïö¤'â/?Is=̟?R¶ûÞ;¤µ?Is=̔4FGL J0221.1+3556¿ÔôÙ.¨mÀ7|K	éÎÀ70–›¸XÀ;)ûbó@Žn F±ë@Çâ'@¸?ŽÁsR]?¨¿3\"ë'@(}@@ Qg`Œ\Å¿Ì/
3Å)j¿àå!×¿ågûý<a¿âý§*{ԍ¿èKABG£¿ãE5þAGNFSRQ3FGL J0221.1+3556B2 0218+357?ïùó·	-´?Bð«?H1#ÛI0?Bð"?ïùERus–?`ý`Gø%?Jê¶*1¦?`ý`Gø+?ïśÎf0ð?€½½§|5?}2Ì燇?€½½§|5?ïÿÞIW
>éBˆjçZÈ>ðÛTpú>éBˆjçY4FGL J0221.2-1312¿¨%¦ùB¡ÀP4 {5À:ý‰»Ö"À<›óÜ܉@ÿB%¿WC@òa|ÚQ?Æ SG$צ?°¬°L¹l?ä܅§tM°@l6k!=?ã¬X]ºn¿æš·¦ÊÛ¿çuK;gµ¿êUü¡PÈ¿Èò]dŠ¿ïø^졬AGNbcuTXS 0218-132?ïø#¡"	%?P¡Êò#xÓ?Oqy³Ûf?P¡Êò#xÓ?ïøù 5Ö?böoô¢=?L±(© ?böoô¢4? Çâ?†•Òě?‹•wúŽ¬?†•Òě?ïõÉ_mdù?IÔ3îìq?TmA%6
È?IÔ3îìk4FGL J0221.5+2513¿ï0^¶Æ‰XÀ@¨û¼¾bÀ;>1ø .À<Ò2º¥@œ9í±?ûåɾ$"]?Е™"Ë×.?Ú3~݀¤*@
Ô'ܾ²@	G¹¢£ƒ}¿ïÿÿ" 5•?ð?ňP†€7H¿Ù¦¿<@x¿ä"éõҀ¿ïÿô!O…úAGNfsrq3FGL J0221.2+25182MASS J02212698+2514338?ïþ1®''?.û
êÒî?,åÖ÷م?.û
êÒå?ïõ¶ÁCB±?sêŠLے?T'}yzŸ?sêŠLې?îDˆG—®?¢j÷Y]ù?«¿§{†…(?¢j÷Y]ú?ï®6=nöp?r­*Ÿ—¸A?"rp¤Bc²?r­*Ÿ—¸B4FGL J0221.8+3730¿ç<çFLõdÀ5÷Yš¦	À:àÐd1À<m?!Î@iohی@êS%A)?ÒÇþÜ¿^$?Ø*Œ»º«¸?úÔLJémí@Édm<ïJ¿îLAœ''?êÿý¥\Æ¿åº<;ðq¿ãU]Œþ¿ïøª*s?qInAGNbcuGB6 J0222+3731?ï¼ÿ³K?"93¥_¸A?€À9;mY?"93¥_¸A?ïܙH¬Hm?ˆ1ha§D?q³[©ÛÉÙ?ˆ1ha§D?íýŠØ•?žö\¹û?°û©;Sþ?žö\¹û?ïyß0p2?'2½…óº‡?Äñù¾û?'2½…óº‡4FGL J0222.0-1616¿ÉYçû¤`7ÀP—æî·`À:'õˆ­¹À<8Uêî @éÐ[L¬×@GڎVo?¶é9"÷ƒ¿sâX'Ö'?×Vj…YñŽ@
mc-ת?íëw²¿¿åY àŠÄÀ¿çWeÂ|'Ì¿â€3aV\-¿åû]8À:î¿É_A"ÛAGNfsrq3FGL J0222.1-1616PKS 0219-164?ïüQÕº?6§‡g'Ó??åwqR&¥?6§‡g'Òë?ïþ3‡âô{?JIÑEõÎk?,ǁиmò?JIÑEõÎN?ïï…֤Ɏ?`øû8f?`z)[6q•?`øû8q?ïþdÙ5ë?&
P–?)²l®ñW{?&
PÜ4FGL J0222.6+4302¿Õ¨Ò>þÎÀ0Ãúñ€À6¢7Q¥åÀ:°"±"L[@Y³Ã¼Wà?þPKŽz??¸ì^ý*?¦d'‹‹@Og+ˆD@B{Ÿ]©¿ºÆ}A8m¿ØPÜfrÑ¿àtÐ!#~¿ÜÈh¤".M¿â4áô|>?¿ßuAË|jµAGNBLL3FGL J0222.6+43013C 66A?ïü‹)_Y?@«€ÚË??3¦µ?1?@«€Ú×?ïôVW/a?tä[›~3?WSQ¡=è³?tä[›~0?ï $'~?	;xZ_Î?‡öÛÛ`~±?	;xZ_È?ïÿx"D?	KL%(m}?í—}Ý4ä?	KL%(kc4FGL J0223.0-3447?×ÿÝá™òÒÀQ>þqŠ†×À:ù]Ø"keÀ<²Ÿô&­ê@`À"…b@4:<;ðq?Ñ+ºûéñ?Å¥o±"‹?ñÿPÈooú@	û2:å¯?ïË^£#†¿Ó0¿P‡Î¿çšß¿Ø¿çkº=©î¿ïøô=Te¿ï;f›ÖAGNfsrqPKS 0220-349?ïåØêCOV?pAªFËÖì?j'¼°©"?pAªFËÖí?ëZö%?œo¦ñ͜	?ŸÅ)Bv·?œo¦ñ͜
?î]šË'A*?˜(}oï)¹?ª&SM‹í]?˜(}oï)´?îîâ^©—?Ž?)¨Ï7?¡Úf‡	?Ž?)¨Ï64FGL J0223.0+6821?èm
î¯×#@ïÏ_ND1À9ë¼&Œ[ÃÀ<Ê<ϔ'@ —W´?þÉÎeS@ð?¾¨*+!ÁÇ?¹Fho*/S?ûàÇ¯;@E®CÊ°¿á€À_+3µ?¬–ÄŸÊ®¿ã.Ò{bw¿Ô.iàCw#¿âúã±à¿á6YSXmAGNbll3FGL J0223.3+6820NVSS J022304+682154?ïÙ°ŠP ë?qÎàÜÛ%¥?s'º×ï‰Ì?qÎàÜÛ%¤?ïÒYG¦F2?mòäÞö3?vÓ\,Üæ¸?mòäÞö2?ï«4aÛ7˜?"H•Eg;?…2ç‰2Þ?"H•Eg;?îðëӐÀö?‰î›ù7à? ñBÆóðž?‰î›ù7à4FGL J0223.1-1117?Ú ¤);ðÀO¡Ò|96'À:6–•[À<}Hé}Ý{@ f&áÁ&?û*|«LI…?Ëkûf=K»?ª×Äøm?üàÝ%	¤Ä@\PÈðIT?îI=@}H«¿Þ•ØCùT¿åµmÕÆp'¿ ûsÿ+CÑ¿ás~§Ð¿¿æb»K›	AGNbll3FGL J0222.9-11171RXS J022314.6-111741?ïÿMÂ¥?ùä$xi?V_Ç«€¼?ùä$x{?ïýä—pà1?KàHÐVá?0ÛDxþ|±?KàHÐVò?ïç䅋#?rÀ"‹Nÿ?hãztÜü?rÀ"‹N?ï÷3ð‡ß?Ckh‹ ?Q™òðBÔ?Ckh‹¡4FGL J0223.2-1653¿î \êþV¯ÀPœ!ÿ.HéÀ:¡'&цÀ<,:ñm–@aĪêNé@(Fya?ÑéQò;?Ûbs'žÔ@	¬s@i|›@	("ÌUX¢?ëÚ7ïZ–O¿Ù1¥^ɹó¿ê"÷€Õ}u¿í+LŸjéÙ¿ïý—ÛSxM¿Ãˆ´oõ˜AGNfsrqPKS 0221-171?ïÛýšUje?zãËc¶?r2ÕJÍG?zãËc¼?튡f&mp?Ä!·HJ«?³ªôÎ̔€?Ä!·HJ«?ìÉÔ* Ø?©~ŠºDYK?¿i±^®ùC?©~ŠºDYJ?ìÖÎK{ú?¬)>¯ƒ•?¿yI¤ -?¬)>¯ƒ•4FGL J0223.5+5415¿ÛD`š	)ÄÀêÁ5¿ÕÀ;UZ'ÇÆÀ< ×Ê,ß@!níËuì?ú½ý¬h©7?Øy*"é9?âD Á@§@=\œ¹Ë@}µ…]w¿ïä…CÛ¿ïÿêњ'ç?ð?Æ´ž˜1Á¿â¼œW~¿æ¤À>IëAGNbcuGB6 J0223+5413?ïüÖ¿Š?AÖ36Eú??™O"¬D?AÖ36Eþ?ïñáí ן?"ŸdCkC"?\<%¾PÃ?"ŸdCkCƒ?õØ?‰Wqîë)/?ŒQ¿ÿŠ?‰Wqîë).?ïё ñjÀ?kéþÖ8æ‰?w7o‡J :?kéþÖ8æ4FGL J0223.5+3912¿íVÔciº(À4BÁ HàDÀ:†câ'§åÀ<yˆ¥U@²Š}òÊ@¾4[Q_n?ÃGÃx4–?¼b	4‡=?ö®…ÙÚ@¶œ€SÍ]¿ÕÜrÝGÅ¿á‡gÓMðN¿år5a¶©J¿àyêaÞv¿ÞD]·ì¿ïíE]'<0AGNbcuB3 0220+390?ïú<҄Ì~?[/Ô877?GµìÎü?[/Ô878?ïûÃk׺K?]JPلH{?@òP¡ÖÎ?]JPلH‡?ïä¬au<«?xUޟÚY?kSžŠÃU«?xUޟÚZ?ïÙ§Ç?`ðxÔ<Y?s,pòœvr?`ðxÔ<W4FGL J0223.5-0928¿ån>Ç`dÀNÿ‰?¯BxÀ:ã‹+AÍ*À<¥­ç.wã@$£ÞlŽ@×:ÿ°Nè?Ì
,"óŸõ?Í4M¦‹ð@ð÷"0{É@(Ätñ¿ïÿÞ!ˆæÄ?ïÿíáoq'¿ããªÿójÆ¿áTî~ù/V¿é¼êº:#¿ïö…Î
ºnAGNbcuPMN J0223-0925?ïÈ~ëL®?}.þµjb?{ÀóŠY¨?}.þµjaÿ?ïÛÞM"ð¨?‡¤•Õwj?rÙ5‡«ý?‡¤•Õwj?íP}=7üá?£h¼…T?µ|@î?£h¼…T?ïÈÕÛ…?ŒKdÄ^¤?œFåDŸïZ?ŒKdÄ^¥4FGL J0224.0-7941¿ëtrüVÀBAþûôÅÀ:liÁd¹¾À<|Jù"–-@J&>Ù@%Û[ÛÉ?¹Û©´nÝ¿™1¿ìÞ?àæzÕéV@Læ/ŸTï?í"Þ9Û¿ä©Q†¿å
$¡u;¿å¤=ÔÌË¿Óþ_o×(¿çˈ>¨\UAGNbll3FGL J0224.1-7941PMN J0223-7940?ïõ¨â¿¥?N#¦KÎA?T®:€µÒ}?N#¦KÎ>?ïýô	«yž?Fۍ¼çûv?0_²¤3
}?Fۍ¼çû]?ïçç{n#š?nøÏÅT\?h"'Üf?nøÏÅTR?ïó%7ª?IN;̦r?Y鵑歓?IN;̦x4FGL J0224.0-1850¿ËUûñ™GÀPËʖ'§]À:ÚlVjoàÀ<•?†'Í@ gšÅ=·F?ûµ1öQo?̩͜çD?ÑŖb,šé@)à¤&?úæîÄnYz¿¡%uŸ-F#¿ÚRÅ؈?çHšÙ4º¿ÉH‡r¥¿á•îê.¤¿ïÿªÛ
}2AGNbcu3FGL J0224.1-1846GALEXASC J022404.29-185029.9?ïã—%"'??o'‰rï?lhÚlØÀ?o'‰rï?ï»k!®4{?˜ŒÁ5 Á?%7"rá??˜ŒÁ5 Â?îéÏ­ŠÔ?•?dª«øh?¡c5'R¶?•?dª«øi?íúl4.?Ÿ1Æ+"1s?°/C"ž^˜?Ÿ1Æ+"1s4FGL J0224.2+0700¿ê~|¥nËÀH'$cŒ—SÀ:wpoÔ¤2À<F'ŸªTÓ@Rý8$‰¢@êN7›wÀ?Âc\›·V?±áÁ'ýö?îí{ì	©@«ºCf§?À®|ª }¿âÁŠÿ¢âî¿æ'~Ý«—¿ëÙ—Œy ¿Ê
#D}³_¿ïþËí©¼'AGNfsrqPKS 0221+067?ïýüdÇë?.h—ãäÂ?0߁À°Ï?.h—ãä6?ïþG
û?K6#[žv&?.ˏ N÷Þ?K6#[žv.?ïèÔmT·?f<p~Eñš?g+'ñ«GÕ?f<p~Eñ?ïûh†rÔ?7	녵?B_íæ4±Ç?7	녜4FGL J0224.2+1616¿ä±Z!ðÀDü;OagÀ:y–JYÀfÀ<J¶4‹@²($·Dz@jlBHyì?Á=z^ëÈ»?©ËndÁ˜?ê´¯ÕEAS@xƒÚ?ï;2G¿ÍEäßq¿æóÇb¦ÿ¿á"Þt"ý¿ÞÆlÊS¿àÅFÞ	5AGNbcu3FGL J0224.4+1615NVSS J022411+161500?ïè¹ {Ây?]ìœÆç?gF߄=†/?]ìœÆç?ïüc–íOü?RÖÞþŽ?<ãH•€ ë?RÖÞþŽ?ïÕ«ÍvÔ?uç"m•…£?u*sĕè?uç"m•…©?ïÎØYŒ9?b¸)gÆ'?x"Ó9ãu3?b¸)gÆ€4FGL J0224.9+1843?áǾ"gYXÀCn¾H¥‹À:ìxc¾ìÀ<	haQT@wv./"@CEÏíé?Ç`ü" c7?Õ½½eP½@i¬ÿ§ël@¤yÊl˜¿Óp¦{RF¿çF—ɵÁ¿ì¯D]f¿ïÿÿ&¦³?ïÌ"'áÇ0?ìMÃ\á'AGNfsrqTXS 0222+185?ïýˆ• ?;•XaD]?3»Wožô?;•XaDd?ïý]Ò);Ó?^‹qµž<?5n¶!lS?^‹qµž4?í¥Åðk™ ? ðÜ£yä?²ÑÐ|£2ù? ðÜ£yæ?ïÿÈŗŽ|?Ï#š$·>û48Â~á?Ï#š$·4FGL J0225.1-2604¿Éùj´²ËWÀQCÙ+à‹À9xöžWn|À<oKG&/?@f,êįr@ÚÖzËx9?¬¯àš?°ˆ©¡x—?üâqÊG·O@,æyq0¿ÒvÊÍL'¿ã™_÷·\¿æúK '\9¿æ˜§8Ϫ¿ì÷Î8׋¿ïþÊ@*'{AGNbcu3FGL J0225.2-2602PMN J0225-2603?ïÿ©NÍ°?`»)Uo?êÖ&IÁÕ?`»)Uo?ïþ¼óc?>eT…—¤Ì?$0ÎÞùÈï?>eT…—¤Ð?ïáÿ•Žè?mK½ž˜"Í?njqòƒ?mK½ž˜"Î?ïÿVº¶ld? O§Ê?(©2skð? O§Ê"4FGL J0225.6-4502?ÚÐ%ç*ƒÀPNe¾ ºÀ:ËY%5C¯À<niØá®@Ú}¬Þ@ÓÁÛØ‹?ÁÛ«¢Z³U¿`7hÆÕ]?'Ã`Áû@á9|Î\Å?ëÅ3 ïò¿Úˆ€Âˆ%¿èri>‡û¿â?–ƒd£ï¿ë}·PcÅ¢¿å۞¡Á0aAGNbcuPMN J0225-4503?ïù×X"	?D¨fŒ™AÍ?H¢ŸÓwڞ?D¨fŒ™AÕ?ïþ׀Ý(‰??'|{pw,?"‡ò-wxÌ??'|{pw5?ïÂCÇñ/?'¬îná?~Þ?h"?'¬îná?ïþfì.qV?àŠ<'!?)'=êyP?àŠ<'+4FGL J0225.8+1310?•÷ƒuÝÜfÀEÑ¢Æi}À:NÈ.›À<Rû15,@ü'Ñ*T'@üÛ`
†Ñ?Ã7²žÎ6Ú?¿0°Ìæøó?úÆ&Nyá@Ú_‡z¿³ùû€Q¿æ(¾e*ý¿ß=ïN×Ôh¿Þ°JJ¦í?¿âqâE"ï¿ïÿm²æAGNbcuNVSS J022551+131046?ïú¾K´ßô?C@É´~@?EÑ,€*h?C@É´~5?ïý¡åù"U?O|±Y-3"?2ðÐ3Ý[,?O|±Y-3?ïêÀN'?p[Lýùü?eþ?÷±n?p[Lýú?ïî0
Æc)?L–üoâh?aÏõ9œ×K?L–üoâh4FGL J0226.3-1845¿â{ìo2¡DÀPª¼£nÀ:¨"7blÝÀ<l¥Ö¾¾@ p®øU@¡Ðº˜ã?ËÇrÅÅFœ?ÉAóU?ù¿g¤T¿@¬äúëï?ïÊBy!T¿àâՂ}ô"¿é\sÔ
2î¿è=•ø$il¿ïþÁ¦þÜê?ïñ"aÎüþAGNbcuPKS 0224-189?ïþÐÎZÏ?0,
l•Î?.BóSé?0,
l•ö?ïþjØÅÏô?Csd°ÍE?)Rs£±É?Csd°ÍI?ïJ#°wf?ŠÈF-w؉?–»‰ñó.?ŠÈF-w؃?ïü1öM1?3_R'ûRÚ?>w M–m¼?3_R'ûRÝ4FGL J0226.5+0938?×kZMSáÀGMÔ{í·(À:lôI:ÜÀ<a&õ7O"@<«S«MÌ@Yúb1M€?Æ06(°ù?¾ÑGA_Y?úß;ÒDÜ@"˜ÒtV"¿çØ÷°Õu?èά5}O¿ç›©¿+¤t¿Ê,Æ`¢¿ètõ_èóÊ¿ä{aT¯AGNfsrq3FGL J0226.3+0941NVSS J022634+093843?ïûˆ²å'R?C2«;¡E?AÝ4kb¹R?C2«;¡Dÿ?ïýðKêU?J[V«q?1â} ­P:?J[V«q?ï·@ìK°?ƒ£C¦r)Ñ?'/û"í?ƒ£C¦r)Ï?ïÿ'ê'?Q´;ŵ?½èæ?Q´;ŵ£4FGL J0226.5-4441¿ÛãÞà÷ÀP6Þ¹^[À:_Í¥òmÀ<uW¿Úv@ Xûâäç ?ü̏	óžÉ?Áçt†B$?Á0ŸD©RI?ý0 Y;Û@5qß@lØ?Ó_JrÉK¿êС£SV¿¿Ãz
?åH¿ßœ{¡6¿à7#"ú¿äÚséܨAGNbll3FGL J0226.5-4442RBS 0318?ïþ@ñ×ÅÇ?)q´ë' N?+ð⃣Ÿ"?)q´ë' Ô?ïÿ`'"?6¨þ&ŒM"?óü­~Q?6¨þ&ŒM%?ïõaïÅq?^î9d³Â°?Uý< uã?^î9d³Â¬?ïú>EF
î?70×Ù)?GêçÈB«?70×Ù"4FGL J0226.6-0553¿ÓTkƒÀMz
í(ŒçÀ:t`§	Ä¥À<—À{†@ÕüT#î@ä;ÜO Ð?»¹J9	6
?'p%_"—?Ôî16ñL@¥$Yт"¿´¡¢¿å0¤ãy·|¿Þ'Ðý‰H¿åÜv"œ;¿âÇîvjÀh¿ä§­­"AGNbcuPMN J0226-0552?ïú¬°›ý?=‰=j|áÐ?FM=v?=‰=j|áÎ?ïþrPߢ?E+K·¯õ?'(ÚòäÇ?E+K·¯ð?ïæ+ö"Òc?qiWÍt³?iÔ	{-œ?qiWÍtµ?ïüšx¹3?,EfP?;,:4kz?,EfP¾4FGL J0226.7+2312?à:Qï¸P
ÀAS¹bŒ½À:´ƒ*ÂKÀ<aÝ6§[ú@ 6՝@YbÝDê?Â˅úÖJz?—‹|ËW¬º?ÖÏ;üZ"?üà/€ L¿ïRW…øÒå?ïÚî}÷|¤¿ãϱƒ›*"¿äŒé‡îvk¿æãÕAæT]?À‹#õ}›AGNbcuGB6 J0226+2311?ïõ˦,ª?P"w#ù1
?Th³¦Ä®°?P"w#ù1
?ïDzès=?¡?nQ˜cY?|&‹ÆawË?¡?nQ˜cY?ïΒG€Ü5?xBÅ­é»?x¶Ü?'æ?xBÅ­éµ?ï\w"Aùª?…Ñí&r¿Û?"q
wÀÊÉ?…Ñí&r¿Û4FGL J0227.2+3928¿á!‹:µÀ3Áޜ)¦À:Qnf)À<
ÏCŸ'@Ê·Í·-~@ÿëJ?ÄúPþöÅ?£"$à_%Õ?ØzšÛ@
ÈcCqCå¿à«RÿU¿ær»ß>¿X¿ê_«+'U¿âÄC@Çpl¿ïɧ~^ª°¿ïâÁ*ØßAGNfsrq1FGL J0226.0+3922B2 0224+39?ïüïâRšŸ?ISÚÓ?8€ík+g?ISÚÓ?ïþT>I—o?BêßT³Œ?*¼f‰!Š?BêßT³c?ï½EZÌ?ÄŒx4?€®©{ÌúU?ÄŒx3?ïø	7?Aƒ*Eƒå?O¿Ûëÿ#l?Aƒ*Eƒè4FGL J0227.3+0201¿É!h	²?ƒÀJgãŸw),À9­ÑI3O¹À<,Y4©@îÞA>c¾?þÈ;4¦?²D
Ëð"??œÃD¹?ì¤ò'Ð(¢@4>=¨W"¿á¢žA-¿àÂñLO¿àŸÍàÉ¿ØKêd7b¿á‡Û+4a1¿Þ`ø=hì(AGNbll3FGL J0227.2+0201RX J0227.2+0201?ïôýG}â2?Oüœ;Õ³?Vq;›î?Oüœ;ÕÄ?ïüûâí47?S>tà\X?8 è–^Gi?S>tà\T?ïÙæ²Î…H?w5nN¤C×?s¦˜½[Z?w5nN¤CÚ?ïæµ >ŒÝ?X¡=«¹?iJßÁs$	?X¡=«¼4FGL J0227.8+2246?눕'O	4ÀAvÐâ2À:'3"«CÀ<S¯s²M@ïæÌRT?ÿI-U£ "?Ï0šgó
?Ë›Â߁@kq'úä@kÓ}–á¿è‹ïŒë5n¿Öa/šÍKM¿á‹öþÏ~X¿ßØxýlÒ¼¿æѳ¼ZŽÂ¿ïþû=x†zAGNbcu3FGL J0228.0+2248NVSS J022744+224834?ïýå	Ts?1¤:
A¶)?0×µ\gåh?1¤:
A¶?ïýåb«ºÿ?N/ès˜?0Ôê¢(	_?N/èsŒ?ï «å%+r?"µ¸¼€¶c?‡Õ¶µ#G?"µ¸¼€¶_?ïüN[.]­?1Œÿ"
V?=&‹?1Œÿ"
M4FGL J0228.0-3026?Å¢1BôòÀQ'N;Í5¨À;óÜ܉À<·‹"- Ê@MϹ'0¿@î#yÌ?Í×¼w¯d?µ±-œ"`?çؘ²é̸@óÔyêQÃ?êDXŠÑ ¿Ûw"}~[¿ã*l»>¿â³_þÃ?¿åª""Žö(¿å0´hQøñAGNfsrqPKS 0225-306?ïþÔø\/?!ã¹i¶"?"°~Z=2?!ã¹i¶?ïþœÈS»?Cøgxt?&3zÏY€?Cøgxt
è?ïñǂgR?g%häB?]Òpû1[??g%häB‡?ïþH"Ü¿?ç,¬Î¿]?+~6Â4_?ç,¬Î¿Ž4FGL J0228.1+8208?èÛ¸¶e^ô@3뚝¥—ÕÀ:¾R}{UâÀ<\±•+v@je›»1ð@" ß8´?Շ#	ðCÊ?¤k·^%¥+?¬ûŠûF1é@¥CWm¥¿ÖYì x±¿è¿¾ëbº¿ã؊:N¿Ý$þývÑ¿ïÿô╋î¿×·0ÃÂ7AGNbcu3FGL J0228.5+8213WN B0220.3+8153?ïþÝCkÖÑ?!>Wn¶mð?"+ÉB'ße?!>Wn¶n?ïþIõö/?B
?uÛÓå?&+` 
"?B
?uÛÓÎ?ïÑvT!L?~w1è{?wDÕïYòm?~w1è{†?ïýÀFµvE? ¥ÐåUfN?1ýÊTMÊ;? ¥ÐåUeÐ4FGL J0228.2-3102¿ï«×·8ÀQ"gßã*À;C—'h$­À<Ӂ¶NG@tãÞaIÇ?þùúnƇ?Ï2·¸=žœ?Æ@b†2¼?÷š™ÄaÄ@?þ¯áa{¿ïŬý¤†?ëÊGÅwÄ¿Ô
=¥ýÖ¿êQÎ(í_?µÿjXäG¾¿ï÷£:,K¸AGNbcu3FGL J0228.7-3106PMN J0228-3102?ïóZð‹m?fV4–'?YKÄé&?fV4–™?ïõâ=ñ‰t?rj©*?T;"íä?rj©*?ï!Ù¥*ð?"$J®ZG?›ÄËZ½Áß?"$J®ZF?ïÙ}v—ƒh?j¥›#®WÁ?sAD´>L‰?j¥›#®W¿4FGL J0228.3-5547¿Íp¸
f&NÀL9BÜôb=À8$_Ñ÷®ùÀ;c¤¡4˜Ž@Z4!š¯n@κ'®š³?zùà V?¼âW–>ñ@!±>›A:@€yMHÞ?ë°*Öm_¿ÛœEE"o¿ãZ¡Ëi¿ä!»qZ¶/¿é1ÿ×f.¿ïÿ{uÂ#üAGNfsrq3FGL J0228.3-5545PKS 0226-559?ï¡Ò8žW?…!Ž‡M0I?‡ºKqØjB?…!Ž‡M0I?ïçOô‰O?€8ý×Q€À?h°åv±õ?€8ý×Q€À?îoÈ$?Ÿq;Á7¥?®é~¿E?Ÿq;Á7¤?ïíÇç¬l?]Ýæi-ÅÅ?b8Sè"9?]Ýæi-Ũ4FGL J0228.5-2234?ç¾Ì~Y'ÀPã8`™ËÀ;i+Õpà=À<ÎÀMb‰b@")øL‹@Ægeiç$?ÓsšvL?ɵ˜RÇ£?õàèÄ3¡@+ˆª&À?ïÿ-½R†`¿à÷
}—"¿à8ÝA90M¿äesâ¥Ò¿éµ_B…¶Ž¿ïôó'H¡AGNbcuNVSS J022832-223350?ïòŒ,–ºA?`Mf½%õa?Zç¦Ò‹N?`Mf½%õf?ïí‰ëòøq?xl€ÐÚL.?bv
š?xl€ÐÚL/?îW*?¶ä£?Ì6¯ïfƒ?ª\'µÅ?Ì6¯ïf…?ïÖk{;J
?c8ë+"í'?tÊBbZúF?c8ë+"í‹4FGL J0228.7+6718?ïoߔ2ü@Ã2Ál"À9´€JœÜÀ;€R'KÖ@WFbåÓ@j_ºzº±?À$Ù~6Þ?Ê-_Ÿ!î½@	ýfe§@zâ¾%À?ÎÈ2É«Û¿Ý7‹òç鉿é˜#wÔLô¿æ$Ç_¥'¿êaš#Ø¿ïÿ˒:)ÇAGNfsrq4C +67.05?áT‡·|ó²?ÎÙÉl>¯?ÝVð'›?ÎÙÉl>®?á0Uù›?Ów°(—ë?ݟUÕÈÉ?Ów°(—ë?æZ€ø¯?º`n`6U?ÓJþÍÊ£?º`n`6U?æ§T'¬?¯˜Z$Sq?Ò±WÏ°§ä?¯˜Z$Sq4FGL J0229.5-3644?܌CM\+"ÀPÊW)²€ñÀ9/»£¯À<TPâp£@gHûF‡Ï@´ž¢íÖ2?ªý¼¿õŠ?ÀuýG¾Ûs@ݺӦâ@[¥…`&±¿×GÝyÃ:}¿ãº{&Á¿èkZâ#Ì
¿ê>šš¿ïÿö?ŒÝÉ?ïþüà:è´AGNfsrq3FGL J0229.3-3643PKS 0227-369?ïÿXô3–?zóÒ¤?ýAy@"?zóÒ!?ïüna©å?a)«A'qv??ìŒò°Ö`?a)«A'qs?ïy\¶0?—Õ½¯9g?ŸpÔi<™ø?—Õ½¯9f?ïÿ8Þóz1?ŽZŸÐaß?ä!¹Ýž?ŽZŸÐaŒ4FGL J0230.8+4032¿Ôӆ8ÊøÈÀ2€V>Ðö'À9^9ßõž}À;õp­è7@Owbâù4@r9`sÞ?²uFþí|?Áÿ_C}X@
ÔF"ú@´Â%~ê—?íY!…Æ~¿áò•S¹»¿æ­GÌGl¿ç$L£2¿êӆŁ~ñ¿áÉO?ÙAGNfsrq3FGL J0230.8+4032B3 0227+403?ïîWþèst?`
ëZàµ2?a¨ŒŒ ?`
ëZàµ5?ïû^xÛ?X:ŁÃåÞ?Aʇþ"e?X:ŁÃåß?ïj…<G¢5?Š™F6W,Ï?'¯Xw¹L?Š™F6W,Ò?ïþbˆ
?
±ïÁÖ?)×ç/Ãy?
±ïÂ94FGL J0231.2-5754¿êÃøv7 ÀKJGìþ›|À:ˆ׊•ñÀ<›Î ‰ãC@ ÀWH'>?ÿf[~«Ø?¹hgGŒÜr?wôMcS?Á*±"qê(@@œ5UL¿è1}ˆ¿ÔÔBÃI¿áÌoD[y£¿Ú[h¢×0¿áf¢vb¿ÙK¯RiAGNbll3FGL J0230.6-5757PKS 0229-581?ïþÜ¢z_?(R¯‹(?.25ØZ?(R¯‹
?ïþ[ZÌI?Hø;¸jnÉ?*J^³;ˆ7?Hø;¸jn±?ïõà/I~Ù?aüs"z³?T?¡mMv?aüs"z§?ïüe¥¥s)?/¸Mk"y]?<ÒÒÔfÀ(?/¸Mk"y4FGL J0231.2-4745¿çu}œF2ÀNÑ}àÖo
À9¼<ÛR¡ŽÀ<wš‡Ö"·@W´.o˜@(0 ±»Ï?°sHÞ&wŸ¿—ápa«°a?×·ç"
›õ@LJڪ[¿ßnÑ"2w¿åhªC5ö¿êB€®I¿æhÈ@vÕ¿êæ°£¡Z¿ÍÆRIÎÖAGNfsrqPMN J0231-4746?ïþO¢"?/$¼Ká'M?+ßî&Â?/$¼Ká'<?ïþp
2½?B"v
ÊTÎ?(ÿO\Ô3w?B"v
ÊTÇ?ïÌûìˆ5¸?}@[{°?y'	»å#Ø?}@[{§?ïÿ{öޙ?m_s·?P$-@?m_s·Õ4FGL J0231.8+1322?ïøB°zÀE^Ž`€sXÀ9@¬ï·³`À;úØPŽÍ@?*^ù4µ@F1!àûX?¯¯4'àçÙ?ªØæ`œ¢ã?öÞ¿ù³?@ʚÒÔ£±?åaUðÍ]¿æ܁u¶e'¿ê±]À¥w¿á¾«¡Ú¿ínTqq\d¿ïù>JsAGNfsrq4C +13.14?ïþån²É?"G<,þ¬?!©"Ól"?"G<,ÿ?ïýûAƒw?Onx(Cû?0%÷ãäLÐ?Onx(Cë?ï£_³ÔY:?… Sˆµ?‡(
é±X?… Sˆµû?ïÿß0Ù ?ÞÃ}T?È3É·±?ÞÃ}Sä4FGL J0232.5-1118¿ØØ&}"våÀN½u6
À;FϐÌk~À<³ãcGP@!#T33@?ø~ÃNžÊ?Ô—d54?ÑøXrÇ?ÿªœ"¤?@Î2eWó‡¿ïÓb³S?ïþ!†ù"¿Ò£*g¿Ç¨·aßC¿àMÛÀ…–­¿ä<×â)«JAGNbcuPMN J0232-1120?ïü¢'y5›?9~6Hž¯ ?:îÄ6S,?9~6Hž¯©?ïû¦ »Y	?j>·–Íü?Ag}›ØH?j>·–Íü?ïÒBÐK:1?vŠÛ;°b?vޗÚbç`?vŠÛ;°b?ïéÉn€5f?X±H£~¤Ž?f6'ʙ?X±H£~¤ˆ4FGL J0232.8+2018¿á>Æ»UšÀBIöã÷‹½À:S»'ˆÛÀ<Hö~vþd@!TƒêÛ«?üŽÛÐuÏ?¼"'¾¶´ˆ?'8W¾}÷?ɸ%õç?þªÿu@ž×?Þ"@œ¨AÓ?µê!ÇP0¿àÄ=ÝT¿Ô¡÷¡Œ­"¿ÚŠºÄ³¿Ìœþ¨çë6AGNbll3FGL J0232.8+20161ES 0229+200?ïõÆSP±k?N?zyK²?TsY^+¶?N?zyK¤?ïü'ˆÑŽÊ?\kτÃ4w?>ùs‰±º?\kτÃ4z?ïè¨t""K?o«M?àq—?gW‹{ݵl?o«M?àq˜?ïėâçÉ?hýF§a??}´ôŒt?hýF§aE4FGL J0232.9+2608?ß<«¢¤;À?eO Ñ1À:ïj'"À<'Ù\'HC@ ¤¤ä%ƒó?ýí`Á
÷«?ÈÀ˜a
[ù?·è>˜A*?îï
'ær@=äÉás?î:¦>Ê.¿•+Êz`ª?ÁéýŠ.í~¿àœ~á\{׿ßµQ†'¿áhÖÏ)žAGNbll3FGL J0232.9+2606B2 0230+25?ïû¯žÁܤ?7º"ÝË!?AA"øm)?7º"ÝË7?ïü[ãLÌÕ?W·hJ"ÜW?= 噙N?W·hJ"Ü^?ïäsÎÿ˜Æ?rŠqë®3#?kŒ1g7ö?rŠqë®3?ï­EÖ9E²?p™Ð3Èó?"®Šq®'þ?p™Ð3Èö4FGL J0233.0+3740?îñá½J'kÀ4ñÁç–|¯À:ç±m˵vÀ<£¦Ç…ò@˜AÖd%D@‰cՒn?Ábǵá£É?ƒ:5ØeC?Ãþv½÷qç@'3úý?ïüp(‡Ç?"AØp!¯¿äÎZÁlœ`¿âü¯ég7¿ÜXRݦ)¿ÝDÉޅÜÎAGNbcuNVSS J023308+374201?ïþerÓ¸?3z©_±"?)¨ÒÄ3'?3z©_±Œ?ïþÿ*.­?9U–œòäº? 
_},#?9U–œòäÅ?ïí0q,Ñ?qEdÈt?bώñÓ/?qEdÈr?ïû/ÍËyá?2²×9õ?C@ÈÒxK?2²×9Ò4FGL J0233.5+0654?ç‡YÂE ˜ÀGøAþ¨,À9Ì$$¢v¸À<8 ŸGX"@þL'¸€@®ÓØYÈÉ?±.Ù\R;¿}éHi·dí?ljÂáçf@
GU6hG?ÄÜNŠ|›1¿ã>åD'׿äÉ)¿—>¿éú)Çy¦µ¿Ñ°Zü$ÿ¿Üw¹à`þHAGNbcu3FGL J0232.6+0646TXS 0230+067?ïüžˆZpi?8".3Ù*£?;½,|»—?8".3Ù*±?ïþå£ðC'??ñëÅÖ?!¥ÀûÇ»??ñëÅÖ/?ï矨º`(?kݵbD?h`WEŸØ
?kݵbN?ïþ^÷Îv?gííÍb?*ƒŸs?gííÍN4FGL J0233.9+8041?±.@V+n"@2­‹`ñ²_À;X¯ð3íÀ<Ïoì÷å@"Ď_|½?ô'ß(#½?ÒÜëû?ÐÄ C?ùƒš¤["{@ªM¤x›?ïù9r•T¿èº'S¸¿ïbË#/°?ë©b>älQ¿à°Ã¢ÆO?Àš2›³¥4AGNbcu1RXS J023428.6+804341?ïùÇðr¨?M¶d·"o?K¤à>5aþ?M¶d·"`?ïóNÅ0¬?€˺ÑWõ?YbÞuž¦#?€˺ÑWõ?ïêzë،?ˆO¦?Œ…aE	ÜÎ?ˆO¤?ïæâÁXô?eMêB€¹?i>§éû?eMêB€¹4FGL J0234.3-0628?³fvhá-ÀM?À	oëÀ:š±§­YÀ<~Ûúg9Ë@ f'úÅÙi?ýN$Öyù?Á´-¼åN?±6ªy?ìÂ7åÒ?úÕAX:?ÐÑ`ûmt"?É
É݄*¿×—?!S¿Ûü›KŽ¿ÜÅ%Ä4ͽ¿éŠýtŠkAGNbll3FGL J0234.2-0629SDSS J023410.30-062825.7?ïò"d¨]?RC˜½ã"^?ZÙ6¯EËè?RC˜½ã"_?ïí¬°½—?ta{™X?bSbOBh'?ta{™X?ïÞ°‹6ü?v¨ƒ9q€?p§ºdýî?v¨ƒ9q'?ïd¢fs…?}ƒˆÅ>Ó?"k¿S1‡?}ƒˆÅ>Ó4FGL J0235.6-2939?æI¢'»NÀPÀØì•ÀÀ; ìy:~À<Ä(Ï,"ž@þ™&F|@~¡ñ?¸''™z¿¼'å XO¢@9µ/ê©@5¬(½c¿ÌéìjÕ·¿é8ÝA90M¿åÆ×ÀEÕͿب'n¯¶¿á ˜%ü¿¥ 6@Ù¹ðAGNbllPHL 1389?ïüÄþÉ`?5"eäû$÷?9Ø	·ÝÄ?5"eäû$ù?ïø•iÊÌ?evW(Z–?MªXÔύÞ?evW(Z"?ïß;Ó¤f?y¸Ë7m?pb-¿L*?y¸Ë7lý?ïòl°­?L=–yò"?[&žýÌ¥'?L=–yò™4FGL J0236.8-6136?ì…2ҙ"éÀI¥`Z³«À9&u =)À<\·ã0¼`@âô©	Ï@ž~Û¨1ã?¥3£E"à?¢gÿÚ$?ôŒ]VlG@³O؀Š¿Ú{?¼X‹\¿à.¾#¼«¿çy!¿mh¹¿á ð¥ïé2¿è%ìIiÖ¿çêªcyAGNfsrq3FGL J0236.7-6136PKS 0235-618?ïþ0Õ?&EÏb]o?(÷®4¿?&EÏb]?ïýx³{?ORëè ?4?§êd*{?ORëè%?ïé È+Ã?ky(ZT?f_7ýÔ= ?ky(ZT?ïÿþ©r2>¬‡px¥‹>¯uhÜ⡱>¬‡px¥E-4FGL J0237.1-0714¿î‡DæÚ;ÀMY>_· À;«ïÌñÀ<×µ?èM\@!ÁŠN"
?ú-½qåö?ՔŒ¿kG?È`:Ó:¥?ó.a«ì@ÁÞtj
5?áîÜ÷½;_¿ËK|Öt+?Ö6¾£>^
?Ú7D9ë´¿ß•ë/³L¿Ù±ž6ò…AGNbcuSDSS J023700.77-071307.3?ïøvÄM»?GRÊ1¼0ž?N'èîÉ'?GRÊ1¼0ª?ïý–¾ˆØ˜?LҋŒ÷¬?3J¹;<f?LҋŒ÷'?ïŪoN+A?zѶ9¼‡0?}*ÈXê_Ä?zѶ9¼‡4?ïðò¥iÛ?SkÚ<9·?^µñ,IÕ?SkÚ<9Â4FGL J0237.3+2000¿îQm=.¿ÀB,{5*"8À:úK‡½ÏÀ<x篷é@ [' NT@úŸ{Zê1?Ä×	&Db[¿v"ÞÖ¥ï?ªq)Ò?ÿÙ¨'{ïæ¿ê†_ô‡Q?¤¥b5æR¿æ;Z^›@ä¿ÚOõ^f¿ía@"ð'?ãT|YóAGNbllNVSS J023720+200033?ïëÓ6óÿ×?`Ù/•>¡ˆ?d,É)š?`Ù/•>¡†?ïõ2þºÒ?sÎC½²
^?Uš‹ò^e?sÎC½²
^?ï—dt>…?‡³è?5>å?Š&âüð^ž?‡³è?5>ç?ïåÇßH¾?`ÞÔ"û+ã?j8 ·Aù_?`ÞÔ"û+å4FGL J0237.6-3602¿æèïêçÀ,ÀPq¬ÄÀ: mÉ17À<}Ötì;'@ ]€‰¨4è?ü²›É?¾a"ðg‡?¦_
ã™ÿ?ér\©NBƒ@
'r—Í?êíý¬i¿æ¯2BGx:¿¹ÐÔÄ=F¿Ü®}†¸–¿äú•þ¦~?M/]»œúAGNbll3FGL J0237.5-3603RBS 0334?ïÿR§îH`?
xrDkãA?«6óþC?
xrDkã{?ïþƒwîT\?A&85´Êp?'ȁº=s?A&85´Ê^?ïü-öš{?A{ʖ§?>O;,«?A{ʖ§?ïýg¢ÇtÚ?%À@ßíÉ?4ÂéÄY4Ï?%À@ßíÉE4FGL J0237.6+0923?s>Œo¸èÀF¨ÁTɅðÀ:XœóÀ<U¹}d¯­@Ij¸…˜@ù½ƒƒ­Ÿ?ÌÆôE·š6?ÆF‹?8Ð?üÙíçχ'@…Öf(¨ì¿£Mʟ\7u¿æ‡uÀ –ù¿á¡Ü>ñ§¿ãB–³5L¿èÁYAºµ¿ï÷yHÁ9òAGNbcuOD 58?ïë˶"ð8?cpåðW,?d4I{Èm?cpåðW,?ïýä2Yxh?H›4È5ã8?0Þm4<ºŸ?H›4È5ãJ?¾JÅ?‰3P°Që?X>mNÑ?‰3P°Që?ïå´îqå?UZp©?jKŽú?UZp°4FGL J0237.7+0206?Ӊßbè•=ÀI'•þÚfÀ;5‰+L"À<±&9O¬æ@µY5¦U@—?úÁҞ?ϵ8ªå?º=»aëW|?íUӌÚn?ÿ"Üj ¿ïÿMR™*?ïüˆFŠþÌ¿êó_s-F¿—Oé¢E¬¿å©Ÿ÷Ó¿ïÿú Âî'AGNrdgPKS 0235+017?ïþ²²ã)?#G©ÐEn‹?$ÔßñÍvµ?#G©ÐEn¸?ïë^—?}b4›»%?dïäø¡jÈ?}b4›»$?ïÌwHJ÷­?s—‹snÌ?yÄ[ڄ)O?s—‹snÑ?ïÏi|?l:þ¾Iú?xy±rKBU?l:þ¾I÷4FGL J0237.8+2848?ÎêYâñ'»À<†E^®âÀ6âб§­À;<éõÒ@÷÷ÈÎæ@«9²©5?‹æ©¸ËŽ?¶NêÆÝÊ@(=îVŠPP@!%U¬ÿi¿Î¾üÀ'a¿àkÀ]RÁn¿åß:Wꢡ¿äp°×£Àd¿è6c¿Bµ¿í(/~ȲâAGNFSRQ3FGL J0237.9+28484C +28.07?ïíš7ÐR?\ۏÈ9¡?beïÈ/®Í?\ۏÈ9œ?ï¸6-©3?›†É"?ÿ²t•³7?›†É$?ï­ü2yº?†gºpkƒ?"€ú3a'†?†gºpkƒ?ïèÿ;"S®?ež/"!\)?gÄk¬S?ež/"!\#4FGL J0238.1-3905¿ï¡menÀP2ñVIÀ:B´½âN>À<Š7Âäì@Ój™üÀÛ?þÛ¬´('?º9@‡Y¦?ªŸbM–Ñ?ò'í"Ó8ø@!O0ï?ÛàÈâÝZd¿Þ"›Ãjxo¿áxkì¸$Ÿ¿ÙáN¹÷¿ånß{ûùá¿Ñ顙Ã5AGNbll3FGL J0238.3-39041RXS J023800.5-390505?ïÿ!fn¼a?FÝãµÚ?Ó2(tN?FÝãµØ?ïþH°ñ¶§?E3~³8?+tð䕞Ó?E3~³8
?ïùð»?TŐèUÕÕ?H?áÀw?TŐèUÕÉ?ïüü
Æ/e?)ÐûO5ž?8©Î"Ò?)ÐûO5ž	4FGL J0238.2+1531?îQ@aîaÀD˜²é̸À:n­\ÄýÀ;ìg
ÑZ@)âøc!@n<c?Ê)^H4Í?Âá
6u?ø¢ê`[Šj@rK¡éõ'¿èe‰&"Ï¿Ýä8Ž¼ÆÅ¿ä
€¡{k¿ãUÌ»/¿í;	Uê`¿äËÀ}‰ÁAGNbcuCRATES J023819+153323?ïî×øÕëà?dÊÀ¨ñ/j?a(*/?dÊÀ¨ñ/f?ïþ_F·tá?E⊶¹?*"ˆ±÷L?E⊶²?ïܨ"á¡?"ߴׯƒå?Ÿ"jïcËà?"ߴׯƒã?ïü¤&?€m?/ù™JdèP?:ÞÎü–t?/ù™JdèÚ4FGL J0238.4-3116¿ïÂrø'dÀP•gÊêt~À9/f±%À;êmÀÍ»	@­ÙY"0,?ý0qLsv?§×Q
3µ¿kä#ü'?Ê]ÜT)@È/¨d7¸¿Ò¿º•'£Ü¿Ü.ò£¡¿Ü!HO$+¿Ú¤Š£ÝjT¿ßß­Ácã¿Å¡gÄ4w×AGNbll3FGL J0238.4-31171RXS J023832.6-311658?ïþ"¶›D'? 4ÝiIÌû?'´–K·Ük? 4ÝiI̝?ïþ{°¢ïö?BMFUÛñÊ?(DõÑš?BMFUÛñÆ?ïòêûvC£?h.Qz?Z*	x¼,?h.Qz?ïÿ¯YõÇ?»îÏ¢?ŠÁG$é?»îϖ4FGL J0238.6+1637?ÅJÃÀC}'Ó"À7¤l[ríÀ:þm'JÈ@(ôï֒@·{|x £?f÷'`¹v?·‰.'dœ@(æOTÑé@!#…k9_¿Àòèn¿Ý;'¢‡(ÿ¿ã7GpxŽ¿âVûŸs"a¿çñ=Å]m¿çÇFê AGNBLL3FGL J0238.6+1636PKS 0235+164?ïð'•Ám?Y'`Ó2÷?^úÞÔ}%'?Y'`Ó2ú?ïÄKt"Ä?''·#¶"?}ÚE¶ÿ?''·#¶#?ï[›¯˜?'™+h"?"Œ
ýA?'™+h!?ïêLƒž?dwø͵g?eã³=|bº?dwø͵c4FGL J0238.7+2555?í_# ó À>üú½ ßßÀ;ÙÛ©¢À<…'e²@!!þ}sô?ÿ¤óÕORN?»äY€¿¤•Às"?ãI›árv@üó€À¯³?ïþvÞ-È:¿ëÃ<?ÌHÿä>>I竿䊗hfñ§¿ÏYm3࿦K_
7ÎAGNbll3FGL J0239.0+2555NVSS J023853+255407?ïþýë~'e?p
çäØ? !Hé«ë?p
çä?ïüWq,‰,?PxšE*5?=Dv›¶j?PxšE*7?ïí,˜øŠ"?d[‡þ6C?bÓguÞw?d[‡þ6F?ïçћíE¯?^ü¶6ož?h.dºPò?^ü¶6o˜4FGL J0239.5+1326¿áFòÄÕ¯–ÀDØ΢âaÀ:ú–xHÀ<là‡"´@û-8¦?ÿâZµX<?Ñ´`YÜë(?Ç#–=áã?óV]Ú¦ª@žÃmþ`C?íñ'QS…¿în16ñL?Æ2ØÅS†»¿áô²YƒÿÔ¿ïÿæ¦Sf?ïþùÛ"ÐåAGNbcu3FGL J0239.4+1326GB6 J0239+1327?ïÿ0¶%n‡?=&g"¨?é;R/
ˆ?=&g"¨µ?ïþéêÿ—Ê?Av…ò$?!aPƒ^‹?Av…ò$?ïIŸ/¤$Í?¦Kï/â?–Ì{f[?¦Kï/â?ïþÿX'ªp?)]™I? 
våXñû?)]™I4FGL J0239.5-1353¿áúK±rx×ÀNÃ3ÁÎl	À;sýþžÀ<we'+@¦œ%.@œløPß?Ƭڝwö¿« 8Bf­?ã#û½{ 2@Ý»´MпÓ
e@¡†¿ë䩘^\¿æÏ€Ü3r¿âf="†¿ïL_ŸLáÛ¿îµ{aöDAGNbcuCRATES J023939.13-135409.6?ïüpÌ©bZ?FVFî-¸Ÿ?<yš´í&Õ?FVFî-¸'?ïà'Üë\s?—<ù¥|˜m?oØ#£Œl?—<ù¥|˜m?ïÆBt4i ?ÔÔÕs?|ÞÅåË/¶?ÔÔÕv?ïõÄQB?HëÊS‰ùØ?Tx÷]ã|Ø?HëÊS‰ùï4FGL J0239.7+0415¿íҚùÝ|ÀH'øã¬cÀ9ƒÇhß½jÀ<4Dé>›@~UñN6@ô±$Йá?±Š*!!ôÙ?°ÃʀÓ`K?ö‡‰	ÿ]@_Ÿ —$I¿ÄE¤¤å}¿èTKç_J¿éó¦öyn¿æûÖƒó?¿ïþ©žttÇ¿ïßÂð|AGNfsrqPKS 0237+040?ïÿ•d‰?ð€TТ?
ºfÛÝ©e?ð€TТh?ïýÆÐXã?MU‹z3¹˜?1Ïñ}8êê?MU‹z3¹³?ïá p6»?j»þÍÌn?n_ðÉC³?j»þÍÌk?ïÿ\÷%Í??gì:c"?a^&l??gì:c<4FGL J0240.8-3401¿í¤'I÷bÀPcˆ†aÀ:øg³À<À–Î
>­@ó"¡ëx@œˆFŠþÌ?¿'t Õ'Ü¿¬lB|?îMâÔv?þ/r†r¿â0'9¿äC#k?;¿åsþwY¿âö?ç̂¿ÜtßzúG.¿Ü䜢7£AGNbcuNVSS J024047-340018?ïözA?Kɚÿ!Q?SÕñ~?Kɚÿ!??ïí7ˆò$?{±†ˆmó?bÈwr
Ü7?{±†ˆmñ?ï׶…ìM?q—÷Þ*?t$½	ñÙm?q—÷Þ*?ïæÈú6?Zý[º™N?i7æÉíp?Zý[º™A4FGL J0241.0-0505¿Ã3k—— $ÀKìØ]ú‡À:±²dkºcÀ<'£¤µW@µ×‡eåb@]OG"=?ÅAæ0 .?Á±Ï…ä°ï?ú\œÓà½E?ÿÈaMw×þ¿ï˜?ǖ,'?îóÕðaýK¿Ýá,Ö!à%¿â2ƒ
¿ä:"DÇ¿ânA§VAGNbllPKS 0238-052?Œå¼?«0™ãýsé?‹]ýƑ?«0™ãýsé?ïه‰ŽgG?'¿ŠŸ¨æÄ?s<;8Ì\ø?'¿ŠŸ¨æÃ?ï¦û%æ¢n?"'+þ2g¸?†A6†Wd'?"'+þ2g³?ï̍ûÖ?‹-3äWYã?Ÿ&n@žåa?‹-3äWYà4FGL J0241.3+6543¿Ø"H²Ìm@éh=;À93?Æ¿l'À;˯bXº¬@ 	G…z¨¾@°Ê1u?°‹lÛ Ú?£^î^(:˜?ót‰Y°u~@áj5¨ÙS?ìtxwàâ¿Î´
^'ӄ¿á`¢' *¿á'æ™ýl¨¿á׆߭¥¿â9LÝ~JßAGNbll3FGL J0241.3+6542TXS 0237+655?ïä	XP?cú¢Ž/r?kîíö§¯¤?cú¢Ž/s?ïìñ
Gç?~3-­«Œw?céò¸Ö?~3-­«Œu?ïÕ-HíPF?{¥•a­*C?ui[‰WÝ?{¥•a­*<?ï*¨R÷E¡?"]às$vÙ?šªõ¡Ký?"]às$v×4FGL J0241.9-1603?ìh\IøLJÀOýüÁrÀ:Õ¦Zr<À<'æ$Œ§C@ Æ*uIƒ,?ù²¶»éOº?ÑmÝÞÂî}?Ãñ¢õŽ?ú4°%Í#@(·'㟢¿ïþ"ÖúÎ?ïÿ×hE¿çånÿ½¿¦qì™­ç¿Öý€^_0è¿ê³Ù¡FŒ+AGNbcu1RXS J024151.6-160339?ïý÷–:óv?)ñø–L?0CN(dX/?)ñø–?ïù5*=g?gÒ[0¾—€?K+»W
gE?gÒ[0¾—~?ﳀoèÀ/?'ç½E€~¶?ƒäÏôL?'ç½E€~¶?ïÞ
'›?c‰>›1×C?pøùzl2]?c‰>›1×C4FGL J0242.3+1102?†ï[å³ÀE¥ÄڐïÀ9¾½¨!óÀ<1Š¼‡@X:þُS@{ÇÜ£¦?ºýT)"
F?Ï+WÝ´>@Έ°=@$'w=N?¿Óh'cëý¿â¤ðñ5¿æ¾ð֗Pê¿êðþÊô¿ïù•¸c‰<?Ú6†¤ÊAGNfsrq3FGL J0242.3+1059OD 166?ïßÿ«R[O?o*¦n¸å?p*VÒX¨?o*¦n¸ð?ïùߺ²p?cf·¤k·T?H6D¥?cf·¤k·U?í)º2"?£-ª
EÍe?·î·ê.nõ?£-ª
EÍe?ïò÷ƒõL¶?MjSÄ)?Zøf—>?MjSÄ)4FGL J0242.3+5216?É;X ùà3ÀÚñˉ֮À9mmþ
\zÀ;²'쮤@3éހ~@_°&£Ø¸?¾ÁCכ1õ?˨]ס'@VùzªÁ@²¨ÑÅÛ?ïÿn	È֞¿ß"]ó%Q¿éßø…–W¿è,ñÀw)¿íA"d~.Ú¿ïóãðµAGNbcuTXS 0239+520?ïÚ6ªŠ?"TZJ™'?~2äªôº½?"TZJ™?ïíȊ)y7?{WÞü‹Ñ?b7uֆÈÇ?{WÞü‹Ò?ì:àb%°?¥~§ãà?¾/8üîÒ}?¥~§ãß?ïd«æO·?z/˜ýíù?"jŸ£6ç?z/˜ýíô4FGL J0242.6+1735?ï蕉Ju°ÀBã4›èÿ2À:8.©`¶úÀ<-V@½XÛ@y÷šÖ°{?ÐÿR©úe?Ö‰bÙ?þåä`gHä@;ݹ"¬?ʲî)hÚ	¿Ö¸Éà‰B4¿á^'ျ¿åQ)=f¿íî6ߐð¿ß¡¸¡òƒ–AGNbcuNVSS J024248+173700?ï¨âá	?‰8å#­ý?…ú½G½­?‰8å#­þ?ïý(ìdO?O$ƒˆÜ?6¸œÝ‡G©?O$ƒˆî?êå¨HÌÖ?«NíæmO?Åøi^Ü̬?«NíæmO?ïÕCàM?cvyóŠ'¶?u^Ù}g?cvyóŠ'¶4FGL J0242.9+0045¿Ã¡cé—8¢ÀI¨	ÃÎ ŠÀ;;éÿãzŽÀ<¤§:l™@±)Î/£?ÿÚ¹šû?ҏ¡·uM?ÃjÔL?ô˜çÂòXx?úiè‹Ï×?Í$Cy|n?Í0"W=(ª¿â~Ȃ=¥¿Ì­W|Ë	¿ïÿwy´!?ïõgÉÉãAGNbllFIRST J024302.9+004627?ïïÚK[?cu"+¸&R?`û%´å£ê?cu"+¸&T?ï·£½$0E?'x
Ž@?'¶óîÁ?'x
Ž??ïg]nˆ¥'?Œ½ä;Žr‡?"R.ëO¡?Œ½ä;Žr…?ï,dÛ½ÐH?Œž&öÚÉÐ?šsdˆEöà?Œž&öÚÉÏ4FGL J0243.2-0550¿ïۑçÉÀKø§Å¬GÀ:Y¹'†¥¡À<aß 'á@|7ýÈBO@Æ<ÓG?½nÊc?"KtÈ~ßY?Ñ÷œ§@ @1|ª¤¿°àøûÔÍ¿éÔ¾³¯o¿êx/â縿é§ã¿³	¿ïÿúVrÓ\?ïÿânÁŒAGNfsrqPKS 0240-060?ïÿÕÛE>úÂM;xî>õ]@tT]>úÂM;xí³?ïþ•õh?Dbíâg?&¨°©•Ÿ?Dbíâg?ïé%yió¤?bŸSÞ¦ˆ0?fچ–[?bŸSÞ¦ˆ.?ïÿžë¾¹?Û£Ãü<L?EQ¿3	?Û£Ãü=‹4FGL J0243.4+7119?ï7ü"…"@$Ȓ‰ÚßµÀ9¡¬JvE×À;àf$ø
@Åo!JþV@-[h¢×?´˜Áò#?ª_z@ò'Ð(¡à@›ÅB궿ïýQœI?ïþI|JÔ:¿à­‹ßÙпßÖ³jû÷]¿æ"…€‡ú¶¿ämNí£ÜéAGNbll3FGL J0243.5+7119S5 0238+711?ïúµ@ñŒ?IÓé/üƒB?Dõ*ü9Ôe?IÓé/üƒF?ïðÙ¹"à?sÃZ‹»·t?^MԌØ=°?sÃZ‹»·s?ï~üXÿ(?‹4׆__? tþ;?‹4׆__?ïñQmš¤?R$%	‰f~?]]$Ê·É]?R$%	‰f}4FGL J0243.7+0321?çø"yXô§ÀHœ¡ô±îÀ;V¨°ÑåÀ<¬…\ '@H.ï><@šMô™?ÔçB.x¹O?Ófæ~y­–?üõO؅g³?ù¸0—!š¿ïÕv‰Ê½?ïÿEZ}$¿âîGÜ7£Û¿Ø8OfÆ¿ïÔF"
q¿î·N: AGNbcuPKS 0241+031?ï±sÆ< "?‡±¾W£b?ƒ£p÷÷X?‡±¾W£c?î½lzÚo?·"dBñH?¤)8RY?·"dBñH?í•"¹OýÝ? Ò %ÌFñ?³Vê5€? Ò %ÌFñ?ê¨r<iK'?²FèlÏiD?Å^7Zѹ?²FèlÏiD4FGL J0244.6-5819¿ÙàšC‹œÀJ‹ …±…À9º'‰)ßÍÀ<0?\6a¼@ ‹'6û"¶?ûÜ ý¦‰?±
Þoú?¦å|."£?ø‡¿|'2@
€†µ‡Œ?ïaL'HD¿á§©Ý^•b¿Ö#ø'Äj¿ÖH:	ç
¿áÈ4ˆ¿ª'_ÁåÕAGNbll3FGL J0244.8-5818RBS 0351?ïþÿC1¼—?áe?¾€v? Ìä6û?áe?¾~½?ïþ;NÉg?Iöê¼bƒ?,K"i‰G?Iöê¼b{?ïó´~[5?o釋‰ø
?YʗI'õ?o釋‰÷ü?ïü¶´.Ã@?+͏°±›¢?:J^‰æY?+͏°±›×4FGL J0244.7+1316¿ë6ό£@ÀDÍ_™Ã‹À:h¢À‰ÈkÀ<+ò£ +@¢|f-@Œ°Úþ¾·?ÔR°+¬V?ÐVMênžC?þ¼g#û‡Ë@
Wxelì¿â^lg1g¿ã5V=ú6'¿åɓAÄ¿ç?¡k2Ë¿ïÿyݼ‰3¿ïûfKŽtAGNbcuGB6 J0244+1320?ïúš}<t~?F?†°bH'?E–.A?F?†°bH›?ïûÐôˆ]¨?]HŸ"ïA8?@¼-މ[Ã?]HŸ"ïA;?îhž¼WÛ?›CäŨ¡?©~æ:'g?›CäŨ£?ïáò^;Œh?_OxW6?n
¡Äs˜?_OxW14FGL J0245.1-0257?î¨Ú&æ"ÀJÏohیÀ:B˝!äÀ<oNÇ
p+@ޙÙ/†«?ÿ¨×úþ8?¿uÁ"I«ñ?¾8œ(À@ý"$½@
ý
ÒÁÙ¿¸ª½¬s?ï]&š¯™¿Ó86¨¿âѤÆôF¿á4C~"ë7¿à¯3ß«v¼AGNbllPMN J0245-0255?ïýz.A×h?0·T¸°ÉÌ?4.ñD½?0·T¸°Éî?ïýÞ®8Ç?IJeÒz}g?1
9ˉ?IJeÒz}u?ïÛ-ijä_?së#ÿ-ý?riKJÐH?së#ÿ-ýv?ïøC+9?@wºÌ/¥Ÿ?NóãSÓ$Ý?@wºÌ/¥4FGL J0245.4-5950¿ìÅçÁ"ÀI÷\¿ôw6À;#£Ï}5À<ÏÓ¦Û¡|@,¸aúœ?ýQ3~²†?Ò7'ßm
u?Ó¬ œîã@1õ`iÍ#@ñ_	zÓ¿éÆk>'aí?îþQ>¶ôô¿×3ŠÜgtƒ¿Ø§¢Æ¾ì¿ê¨^=¢ø¾¿ïò'šx¼ªAGNbcuPMN J0244-5948?ïÊgK\ÀÅ?vñ?uΫ
?zÌZQŸ`?vñ?uΫ?ïïL6Uq?xÔõ|½?`â³Éª'b?xÔõ|½?î(ìÒÙÉ?AÆMÆ?­q2Òcoä?AÆMÆ?ï-TlH+£?Š«ÁvÐVÛ?šUrvú‹Æ?Š«ÁvÐVÛ4FGL J0245.4+2408¿ïmeÂÖÀ?ÐaAcwŸÀ9«Ut¦›
À<ÁJ¸Šö@>ÎË)´"@._#|?µtîêXùÁ?´ý"€¢6?ø'"d¦rÆ@¸øU'¬æ?ãºO¼Öµ"¿äk^R›®G¿ë¹ÒߋkY¿á²¡bÃÝ¿è"£Y5ü¿ïöŠþøïAGNfsrq3FGL J0245.4+2410B2 0242+23?ïþ¢¦Çè?-c[ŒÖ¤'?%Փ)Å?-c[ŒÖ¤Ô?ïþv?Ô³?Dµ–h?(œ´Ï†?Dµ–h?ï«Üè¾ÙU?ƒœh21j¹?…ÅÐIªè?ƒœh21j¸?ïþ þ±þ?ÈÎD¿x4?%ð"à?ÈÎD¿x 4FGL J0245.5-4502?Üò61<2ÀN‡|í'hsÀ:Ð$qÏP5À<sóëõ‡@æ•â@÷ퟫ+'?ÄX½L&I¿°Ôí=ì°Ô?àíX]'@Z¹D.Ù¿ÂÁM½£7¿è>}i7Q¿êþdŸg¿ît¯45'²¿§".ÜÈ~›¿Ô CVìÌAGNfsrqPKS 0244-452?ïÿG
+?'CVŠ'?Z›N?'CVŠA?ïó¯dØY?söA'$ÉÏ?X¡Í6ORU?söA'$ÉÎ?;Vä?‰Áχv¹?‹±?*FË?‰Áχv¶?ïüAƒ|™Ð?6'Šº/[È?=óä1¾?6'Šº/[²4FGL J0245.9-4650¿ßå—]Z'ÀNàC¢@À81Êx^¶oÀ;¿Œæ,ð#@­{MÔ@w¹Z)AB?¡™ÿÅój?½Vö†Úz4@%4z[ñ@0|o'4¿Ðnb×Vi¿ám=¾§p¿æL"üÅ¿ç}Ëb>Ž†¿éÖt€Û\³¿ìûgPAGNfsrq3FGL J0245.9-4651PKS 0244-470?ïïg ƒÏ?f!ªãýd?`˜ßp|1?f!ªãým?ïð@ìiÏ?€cޔÁV?_Í~',aÕ?€cޔÁW?ï¼k|A‰7?€–Š¦!s?€å d?€–Š¦!q?ïý¢Åª˜ñ?(,óú
9,?2éÒ«8yÐ?(,óú
8­4FGL J0246.6-3348¿ëþ‰¼cÀP–=Ć­À;Òh;R¼À=ØL\Ïå@!«5MiÀ?ó÷ ›šœ?é£,àˆÁZ?֍˺Óûë?ë½Pù׳@¿¼§»›L?ìoè%ç}¿åú9¢8#³¿î†9[e?àçŒ Š9)¿Ö‹ 1¹6¿ãÒe}ˆAAGNbcuTXS 0244-340?ïõ®¾ŠH?SäæÊ3Í?T£Ð'ënW?SäæÊ3Æ?ïý~ôz"4?OT$܎ÊL?4\.îX)?OT$܎ÊO?ïšRíkß8?‡Ø¾åúß?‰kD¥1Æ?‡Ø¾åúÝ?ïý~B"·?3X—.ܲL?4
ë_ÊH?3X—.ܲ"4FGL J0248.0+2232¿ÇŽW`ã‰À@r9¼º0À:ތ]pô_À<]ÏX˜GŠ@ }¼Î§îF@1jWX?ÈS¤|Ü?£ËF¡
bk?á(2F@̲-9I"¿äDÌMKn¿â՝ÖÀ¿äj‹Û¿à²Ál!'¿Éµû$#ë¿çÓû?PøÁAGNbcu1RXS J024800.1+223136?ïüœTá?1º€g£‡?;-Xó™,?1º€g£s?ïýåÆæ­1?N5óøµ]?0ÑÈʖtÇ?N5óøµN?ïò(v#‰?cÈû¢\ٕ?[¯¸ïÞ?cÈû¢\ي?ïñQxœ?OÝíòÍêª?]]ÇóÐ ?OÝíòÍê¯4FGL J0248.6+5131¿êñ>øíÀçX}o—hÀ9NÎþÖ4UÀ;ÎDŽŽoš@N°A¦¾p?üçC:è3[?³YP¢"Ð?ÀÌê(þ&@©NBƒ2O@OZTŠEê¿á©åan/¿ãQzç&ë&¿ßÇRÅ؈¿ÖÔµÏZEÇ¿à=ÁA(iV¿éÊKéžtAGNbcu3FGL J0248.4+5130WN B0245.0+5118?ï½K1ÝÎ¥?"4]
X-?€­3ˆŒVç?"4]
X-?ï9KÞ!#?´0°tè1*?˜Î";ۙ?´0°tè1*?îèîC(ìF?šéIßu?¡qÍq;"?šéIßv?íÙ^€ß?˜prϬ")?³I5ù	?˜prϬ")4FGL J0250.2-8224¿ïû;>UK8À@Ӗ¿Ê…ËÀ9Ô	:;e1À<K›•ó@ŒGœÌ©ç@ÜÈÞ*Ã"?·'Ž zÚù?¯Åìûw?ó«TA ´@@ŸÇ™‡%#¿ÖÌ`it¿æõ®j}¿æIRŸ48A¿êA<ÀûˆL¿ëM'Ÿ'ç¿ïîxžwNìAGNbcu3FGL J0244.4-8224PMN J0251-8226?ïÿ
ð?Øâ÷?\Áé"?Øà˜?ïþ$mTgÀ?Lµñ&2Β?-¹*¹ƒø ?Lµñ&2Îx?ïã÷m¶Ç%?ph‡({?l'I8Úä?ph‡(€?ïÿ±,™n?Ý¡¯®?©ÚlÒ=Ë?Ý¡¯ë4FGL J0250.6+1712¿æ¾c݋›îÀB‰‹`ñ²_À:àϹWÀ<*v­ÜF½@ ´¹‹Q'T?üB # –x?¼H%)Û?®Ÿ
át=ƒ?òÈ¥‹?cÃ@Ë:¦o¿ÓÏ"'|¿å¨HÞì	(¿Þ'1£X¿Ô¯$f‰¿á™Ÿ]þ¸Ø¿ÓyA쉁AGNbll3FGL J0250.6+1713RGB J0250+172?ïþï='o"?Jûµc­?!&éÁ@?Jûµc®?ïþ0ÈC,'?FãÅÛóbd?,ó{Í6ù_?FãÅÛób^?ïøº¨`?V²\?V¤?M…_¶~·?V²\?V¨?ïùš$š‡è?:ò?I—m•à^ñ?:ñÓ4FGL J0250.6+8435?ïŠßŽ‡@6ir%·I®À:	L‰EŽ€À<~ÿÕ7ÕY@zR½'¾?ÿ¾Ø»gJ?½{ ¡yüŠ?¹íߨ,ì?ý<<& ûù@ð"W_´?Ë©©\/UÙ¿áe'¢xæ¿ã¨üþÿ޿כ#¿äÆ÷ µî¿ïÿ
!ANAGNbcu3FGL J0249.1+8438WN B0239.6+8423?ïý1¢?5TAmI?6w§Bñè?5TAmV?ïúI
Ëûè?d¼tæÚ.?FÛÔÐY­?d¼tæÚ5?ïíC~q?jÇ/‡êz?b!~?jÇ/‡ês?ï§ã‰¥ç?n:Zí-ã?†–†9Õ?n:Zí-ã4FGL J0250.7+5630?ém<«Á}ÀíÊ"Îa"À9ÙÓr²À;çÙÉ4'Ø@ ˜ù(öCi@Büý@´?¾2ÿܙžw?¡]¡à~Ê$?á/¯4_?ôlÃk$;¿çë«_>ÔÒ¿Ûï—<M¿ã'#? )¿Ö2£uæa¿â{ÒÿkÛp¿ä	•ª÷ïAGNbcu3FGL J0250.6+5630RX J0250.7+5629?ïàBÍq2?gÅ3²?or½2ŽÍ¼?gÅ3²?îñĞϵÓ?·¬-eþ? ã¶¢Ë?·¬-eþ?ï"ßLWQr?†ûñ¿€c?ŠÈ,ê+£d?†ûñ¿€g?ì~÷77•8?¥ì¼‰¸iâ?¼FFCV:?¥ì¼‰¸iá4FGL J0251.5-5958¿î½Æb ÀI¥£3vOÀ:ËGxd•¬À<»É{´Ú@øTD«@ÁÅàIS?Ç)%=QD@?ÃzO|jÝ?ùͼì"øù@

yæ ¿çOÊB®Ñ9¿åm÷T_Ó¥¿Þz&ÂaŽæ¿á°.fDØw¿æŽ"¬Ï¿ïÿ¤?åÉAGNfsrq3FGL J0251.5-5959PKS 0250-602?ïý´M%y?-H9Àãc?2_–Ô;‹?-H9Àã8?ïþC&G¾?Ix´SÛÔ?+έ›"$V?Ix´SÛ¾?ïÖFêöß?z#Ó«?">?t܊"üè?z#Ó«?"<?ïûïÁ\Ä~?2©üœ	K?@@úŒî??2©üœ	;4FGL J0252.8-2219¿ç‰ ­•Ü6ÀO£n.²À7ÐUÑì"À;¾t{'H@²«Yà@òþ½x?"Ð-'Å?¶փ¯Íc@ãrý›¢@XxPô4¿ÅÖSeª)¿áãА俿å¯>Õ'å¿æ—cÉÓô¿èâ­[µ³¿êªàHª"½AGNfsrq3FGL J0252.8-2218PKS 0250-225?ïò]òTâ?U_ôq¤'X?[áDV>E?U_ôq¤'a?ïôÜ6n%¾?n¹Wï9?VG"#´ƒf?n¹Wï4?ïÈ7ä¾¢Ä?€6ÅóÏa1?{ä
 ®·?€6ÅóÏa/?ïþX³W_? Ù&4/‹¼?*tʎj%Î? Ù&4/Œ4FGL J0252.9+3834¿ïÝê	§®À2ipÅdùÀ:[>¢Òþ?À<YNÛʗ@Ïa&
««@%Ä'â?Æ"?ÃYí\9fÔ?öȍ$@Q@àÃA]ÃU¿á¤1£:á¿ä´|ÿ…ä¿èE¢>Ù°¿è3ªÇÜ£¿æuI"ˆÁ¿ïñ$€	AGNfsrq3FGL J0252.3+3830B2 0249+38?ïúüwÑÁ`?Eb5ßµœë?D ¸ú"|?Eb5ßµœÒ?ïúïÿϟ¯?eµ"÷Y?D@ÁF+?eµ"÷]?ïº?sXpx?}ýGˆõªh?p#)ãâ*?}ýGˆõªa?ïÝí¡¼é@?a8zfn?q	/!‹`?a8zfi4FGL J0253.2-5441¿æ'
ÊGn-ÀKR.±Ä2ÊÀ9®æb IÀ<†Õ™úèi@È܏ú‰@åZ'"Ã?°uuøՔG?°óéœ;_}?ø=Žkh-ç@¯³ÏzÒ¿ÛN0¥lÕ¿árç]ò¤x¿ç»e4Ù¿éIiÀãàe¿æÇ>îRX'¿à÷ÍaGBµAGNfsrq3FGL J0253.1-5438PKS 0252-549?ïÿxllù?䍍úé?òòaP?䍍ùþ?ïþ"ñ‡?@.7`}õ?'°çŽÂ÷?@.7`}ü?ïãÑ/lbù?l<qc«¯¦?l.Гû?l<qc«¯²?ïÿÊêšM?>ñk?§xÍ>úŠ²Ù`"§>ñk?§zs4FGL J0253.2-0124?æµ´ZNêuÀI‹Z ÝÆÀ:s­<
ÍHÀ<xåÕ²Nœ@׫¤^º@X¿ÜúAz?¾1Ò55?ž•AÆü?â^˜?ü4'g"#?焝=èîÁ¿ÀÆïh-:÷¿â·#\=¿à"Ñ~7hw¿ä	ˆ>þB'¿Ñ6¯ÿâxÜAGNbll3FGL J0253.0-0125FBQS J0253-0124?ïà2gäÔÒ?eóE"Ç??o͘+/ž?eóE"Ç??ïä¨Ñ &û?yJ)
}WÒ?kW._Ù{?yJ)
}WÎ?ïÑb†œò?z¨‰_ª?wN¼ý1†i?z¨‰_®?ï|§a´?y8Ž$©d?~ëÉ}ÿ?y8Ž$©c4FGL J0253.5+3216?ï°yT^xÀ7ÝÝãu…¾À:LŽ¶È¥À<VU°5½Q@°uÔ@9D$>û?»
Äv)?¢äž5ñ»?ç\V­‹¾æ@N;Qkƒ¿ïý‰-:Ë®?ïÿËA²Q÷¿åü&¡ÕRW¿âå`w9¿Ý-` Ô¡W¿äƒ«ñŠòAGNfsrq3FGL J0253.5+3216MG3 J025334+3217?ïÿµ·ySÖ?'ÊIdþŸ?'!«
'™?'ÊIeZ?ïþúa|]Í?:ëµØB|? Yè:#9•?:ëµØBn?ïáy_ßf?r`‰SGá?n† ñ ˜û?r`‰SGò?ïÿ·Ö'¿@>úôÖ?¢'?
v/ï@>úôÖ?¡ýµ4FGL J0253.9+5103¿í‹K߇úIÀ¨—š¼À96Fñ'À;̯,¨Õ@Ä7B·`@‰Y_í¦a?±Q
¸Á?¯†ë8üv?úôš ¨4@×ÒÙ+Tí?înŽ¾tDu¿à7–oB­ú¿è"ÆÜ	¿âù'žªz'¿éI^]®[ó¿ïÖýÓ*	AGNfsrq3FGL J0253.8+5104TXS 0250+508?ïù‡kU`R?C¬× d¾?IâRª~¶ï?C¬× dÍ?ïþh'_|?Gt‰•
}?)öê;W?Gt‰•
§?ï'dA"Eð?… òáX'?‹¦ïšî"&?… òáX)?ïúÉ"¹_ƒ?5Q<'j?DÛuò›?5Q<'"4FGL J0255.8+0534?ëTìªCÀFÉ2µ^ñþÀ:½âïÙÀ<K4-@&ž'a™£@Ø8 þ?α^œÃo¬?¼µ‰9O,
?ñ£ø,Ìç¥@ªdSç‰?ҍyYˆ¿çCÞ¡¶sš¿áå­é¿¿à°
fóT¿èžP¸7ï¿è­ŸÀ¥!7AGNbll3FGL J0255.8+0532PMN J0255+0533?ïüÙ¡\ûå?:êÔ£*û_?92õ ÜÓ?:êÔ£*ûs?ïýÏ=¦§'?G<SßãA«?1†ÊÃmg?G<SßãA•?ïì^©ã?o==¼ö!Õ?cí¡Vâ?o==¼ö!Û?ïêFxñèi?Tûø¿ä?e¹‡•ð?Tûø¿ë4FGL J0256.3+0334¿ëÚ¾¿rOÀG}BÙÏÀ9÷íPÐÒìÀ<AåçP@Äþ¹®â×@"2A›«Ã?¶Œµ°{ˆ?'YÿáÞ=?ÝG!&Á4é@	$¼¥BÉ?ïû†ô{g¿â¤'ýuE¿ãÖÂ^ß´[¿ß3Žµâ¥¿Õú}¹©"¿ìÒ¯/-5AGNbll3FGL J0256.3+0335PKS B0253+033?ïþéŒf]?'©ë<ü?.ñg9š1ð?'©ë= ?ïþµ²¼6Ú?>u–Ȫ"?$¤Ô<'<|?>u–Ȫ~?ïóBØ£&˜?e2Ñ`5
?YzN¹²Ïú?e2Ñ`4ü?ïû—8àpœ?2OÚ0`&?A£~=Ž=?2OÚ0`4FGL J0257.0+3358?ïè.ÝcÀ6K<>t°À;ëÔÏÑÀ< ˆÛ¢@ Qg¢P¢Z?þÊTg`aj?ËY
Þ*m<?ÄGøý'LK?øz_\†é"?úW|5°'?ï'سiy¿îký^åé~?¾Ð_("ƒˆ¿àEéÞö!ÅL¥Ë¿çžÑ'ÙAGNbcuGB6 J0257+3357?ïü¿:ÂX;?9O¨õ›?:)í>0>?9O¨õÎ?ïÃR¿fúd?—⣹,Ëi?~V L'ÍÛ?—⣹,Ëk?ïÒBÝ;+È?w—0•"û?vޑbj?w—0••?`ý§?'¸Äàüñ?¥9÷ %s?'¸Äàüñ4FGL J0257.9-1215¿ã_N5å7ÀLmîËûµÀ:6¯-•À<tÞë³Aá@ß?@1É@oœp
¯?¹Þ!
j¢?"h|ü*?ÕåFÁ/Š²@Õw®bS‡¿Úƍ«p¿å¯¿üò¿è…xDµ;·¿åP½Š'¿êšÏ>—"¿ïÿ€^	J¬AGNfsrq3FGL J0257.8-1216PMN J0257-1211?ïþËõ'Ìî?9FÛüÚ?#@­ƒ1ú?9FÛüW?ïÿ
歜?;ïž;?\ã*L‹K?;ïžH?ïí;/õ?drEà‡^Ò?bÄæãÐÂ?drEà‡^ß?ïÿ%ô&£v?›ï?A{+'?›ïŽ4FGL J0258.1+2030¿Ö¾»ä`5À@ªé>›AÀ:k$-ܲÀ< p­E£@x¾'²!?ÿa­ê‰v6?Äðª7 ¨—?Ïuéüˆ|;@WÚè'®@	úâ"tt¿ïþsÙ°k?ïîQs	?À#^~æe¿á­:*ž9<¿æ¾J''?¿äûF'+½ôAGNbll3FGL J0258.0+2030MG3 J025805+2029?ïãÊjfÈq?jQ[Þõo?l5•™73?jQ[Þõu?ïöì­j
¶?r9§Úÿ?R&¥+ê'Ù?r9§Û?íҏZOÁÜ?¡úØ'õ&?±k…-ñ?¡úØ'õ$?ï">šÖÆì?y*'9«Õ?‹0YJND¼?y*'9«Õ4FGL J0259.3+5453¿é'J™=ÑLÀ¡!MW¢À:Œç='[À;́I@»²@ ¹zæ{¯@È>{?«¡ƒóÀ¿¦z¡÷Ùb?ç¥F`Œ‡¸?ñê2]ö*i?îpÿ¡á;Å¿ãçOš¿ç}îãx	ý¿ë‰ÝÏSÊ?кý Ë¿ßÎ59©AGNbcuGB6 J0259+5451?ïΕA€D?ƒ€Ðtç(?xµ_t?Ýü?ƒ€Ðtç(?ïžÁ҃¶Æ? Í-ÄÚ6?ˆO‹_N«? Í-ÄÚ6?îÚOP±6?•ÞòF?—0?¢^Û
ôì©?•ÞòF?—,?î=ɵÅÝò?¢{+!?¬#d£¢ ð?¢{+!4FGL J0259.4+0308¿è*â-26ÀGbŒ?>qÀ;zVÞ3'À<¸ÁDŽP@"uE?¥1}?÷è»ûÄ1?×›Á''?Áº	戶?ê&¿AžÛÎ@Œú–Àn¿ïÿ`Ï‰@?ïÚ ri¿ãÛJ¾ëԿَK½m´9¿×QmZ÷Gu¿Å^eYAGNbcu1RXS J025923.7+030736?ïÿ.arÁû?s킉â?3ѧÀ•?s킉áù?ïý¾[wa?P1N.~®"?2½$DûÝ?P1N.~®‹?ï⭍ÅaÛ?s~v HE?mRr:ž%r?s~v H7?ïøý†Ø?DF‰Ja?L	çÿН*?DF‰JS4FGL J0259.4+0746?ë®é³™çDÀE¨×¾˜V£À8¦ºò¯µeÀ;—ïrBÓ@qieŸA#@ùü£T-?¥½'&?¯Äà^ô"@	ž>^à`(@:ÍûXü?ëÄS­úпÞϸ$B`¿ã1¾Ý`™¿âgM"—¿åÈ×tÆ{z¿æª ¥gAGNfsrq3FGL J0259.5+0746PKS 0256+075?ïý¼½üì™?,~.£™"?2›8C?,~.£™v?ïüøÇü#C?MOAÛ!-µ?89Àåò<?MOAÛ!-š?ïÖSMÂ?X?v¶ø$
¥?tÖYàT‡?v¶ø$
¢?ïÿéAc?9¢&Öt3?ž'×Ӓ?9¢&Ös}4FGL J0259.5+1924¿ïžÊûÕR®ÀAÒܱF_À:y–°±
TÀ<#/V/@óôëû@õ
3¿?Âwÿk±?r§Î2s?°nD_÷7?ü€íÑ)Rà?ïl¤nò¿ã[QàG}î¿æ››œ©"¿âk
=²é¿ê4:WÎô¿Ýe5#xU&AGNfsrqTXS 0256+192?ïœ'9Žj?'´à g?ˆý±œe­?'´à g?ïÒz¶F<?'jH¹$Õ?v¤ܸb9?'jH¹$Ö?ï'²ÎðÞ?'BW]Y^?›	¦!ÿÄ*?'BW]Y\?ïi«¤P5?{SpÄ"Ýô?'Ê‹ùD?{SpÄ"Ýö4FGL J0259.5-1705?﬌xÀMcðí=…À;,>׬#àÀ<ªçcQ0@ Ò{ÿ)ì8?ùâwXüñX?Óô¸#G'Ë?ÙAŒ&êO•@¼[ed?þoKº">?ïôGe_M¿î½8À:î?Æk¼f£".¿Óx‹A'¡¿Þx'}sHL¿ïçB.x¹OAGNbcuNVSS J025933-170540?ïý"'9#c?8»p°/?3Ûî6äáÛ?8»p°/?ïÔ!¨F4Í?Z•²wJ?uï+ÜåšM?Z•²wJ?ï¡¡ë´¥G?"Å;¼"ô?‡—…Ö®~?"Å;¼"ó?îúr×ãq?'@ÿÄlš? XҁϸÊ?'@ÿÄlš4FGL J0301.0-1652?ÀÀM-«KrÅÀ; g4À<€îßFL@xƒ/ö@A›@bƟ?Í@›üu[ø?§ê­ÞJ"¹?à÷¦ë@šÐ"Øi¹?—ŠØ>M¡?ï"=ý'·¿çU4_ƒV¿ÝRìÁ´À¼¿ç+=e¼{¿ïúª@/ðÞAGNbll3FGL J0301.4-1652PMN J0301-1652?ïý̓€e}?5UëäGæ)?1"ãüÔß?5UëäGæ?ïþNà'Ê?J[Æ5bIß?.kýƒ`Ó?J[Æ5bIæ?ﳁ~:éÇ?'¹Ùýµ&?ƒ qEŽ_?'¹Ùýµ+?ïùP«"¢û??Õ?÷ß]r?J½Qít<??Õ?÷ß]]4FGL J0301.2+2546?æè}0û À<ŽDR?gõÀ:ö} >ÏIÀ<dX£/D'@ÿÜ0B@ïêÄ.˜š?ÇnšgtÙF?§±U¢ô·"?àÊzw•bÓ?þ5&U)R4¿ç™ëcÉ?ê>zúr!†¿ß)ùc-Ì¿èiU./¾4¿âG)T ¿«-£SN(AGNbcuGB6 J0301+2546?ïó֎3Q?TÛ@Ôï,?XRã™]þs?TÛ@Ôï,"?ïî
ý"B?v%sà?apõݼ?v%sà	?爵â[u?ƒÚ¾fç@?…XG[é"ª?ƒÚ¾fç<?ï˜DYÀ~??xŠZ€h~ë?‰îéàp|?xŠZ€h~ê4FGL J0301.4-3124¿ïë¬íÈ&"ÀN¸G¡A)À:ÉŠ ÒÀ<¼¨¨*V@áÚûä'@/S6L?Ã]:ƒ3¦¡?±ÒIäO Q?ì¼^'í0@QºÝ·¿Ò=?%¯½¿Ñ@{EE¯b¿èe¥@–É¿ÓüνgÔû¿éWÌÊæn¿éõF2ê8AGNbcuPKS 0259-316?ïޑ»X?nPôW0þ?p·r?"TÄ?nPôW0ú?ïö™A*•,?f€Ƶ8?RÍ}ªÕ§G?f€Ƶ9?ïl¬*Ä¥?ŒStñœ®h?'jz§«s?ŒStñœ®c?ïכ¶âÒ?d"ÞǹCü?t2$ó—n?d"ÞǹD4FGL J0301.6-7155?á÷IFSÝTÀDã[ÕìlÀ:"ïÙAOVÀ<Š³Ï¥Å!@'ñÒjÆr@óÕ4z[?¸a=݆.?°¸9þå‰î?ô+¸e6»~@Ÿ®†¨?Ðt=$à¿ã4ÿ@'lT¿åf‰l$ìI¿èrNf•`O¿ì°a¬m\¿ïðȊGìÿAGNfsrq3FGL J0301.8-7157PKS 0301-721?ïú¹	ɚ?B¢›Þ®?Eۼ٘)?B¢›Þ°?ïþ_‹š]?IÞ7ä¹?*FZ.˜L?IÞ7ä¸ý?ïê"iK_K?iˆ­×é?eݖ´ ´"?iˆ­×é?ï÷óì–?=È~K†þ?PÌ'ÈÑd?=È~K†ù4FGL J0301.9-2731?¿%ÜÀNŠó¡LìBÀ:©·¢åsÀ<°XaÀå8@-^g¿Ví@ˆÐâ2?Å.ä —?»œ©'ý?ö8›P˜Ÿ@3êrúôR?ï¬W¿ãž"Ô]ºÆ¿ãÓÂT£ÆC¿áÝŸ¤u–¿ê2ËŸ¿ïÿ3Qf$!AGNbcu3FGL J0301.8-2721NVSS J030158-272754?ïýƒ»¬g"?3ms*ªÚk?3â"œÃg©?3ms*ªÚx?ïýl"£¸?MÚ¤QÊÿ?4žï'â>?MÚ¤QË?ïÝg±!Y?z!5{ܗw?qLp§oSá?z!5{ܗr?ïìì1TaÕ?OÚ/×^ëo?c۞*C?OÚ/×^ëo4FGL J0303.2+3149¿åç[=:À76˧2ßPÀ:hµ}$îÍÀ<@¾(Å@tÙrÍ|ö@i=Š¥
?Å-h±Å4?Än³&ˆì?ÿ»iGÂ6q?ÿÿ—ðw ô?爆ìî«D¿âÁ²‡§(οã%Ɉt®(¿æj}ík¨Æ¿êHuà+ú/¿ïÿùëñAGNbcu3FGL J0303.0+3150B2 0259+31?풞úEÏ&?®7Ì]SüÔ?³k-цÙ?®7Ì]SüÓ?ï3ìLæó&?¡mУÅ×?™'vc!›??¡mУÅ×?íO»Œ?£*rl –?³}'#Ÿÿr?£*rl •?ëÒ̂/?Ÿúî×qö?À´Í÷C»·?Ÿúî×qõ4FGL J0303.3-7913?í…U§`nÆÀAý´þyîÀ:F‹yEf<À<c@þÍÐÙ@rË7@‡¤¤—?½ù
†? Ç†>?ã	Õ×7‰Ú@
€«Œ
e¿Ñÿø^¿ä"\0ýN¿égþìډ¿Ù@ÛýÂ8¿ë¾Ïÿ1N¿ïÿLkAGNfsrq3FGL J0302.5-7915PMN J0303-7914?ïýGÀ³Î¬?6úôgÀŽ?5ÁúaŠ¥'?6úôgÀŽZ?ïþ‡z"?IŒ§™!êY?/ˆ]Þ/¢?IŒ§™!êL?ïêbÑR¨@?o×fbù5ä?e.­WÀ¿?o×fbù5Ø?ïùþ
§Äv?:$ç;#\à?HÕ`î'?:$ç;#]4FGL J0303.3+0555¿â¤æ»Æ¢ÀF-û¹À;Tšù*4À<‹ºˆ&ª@"¡ûï»?øÿø¨ó©°?ÖwºKÀÉ?µÎî:/Ѫ?âºcslß&@bü]^*?ìÈK~ºE¿ïÿòß0&¹?ïþ'¨'Y¿ä«­Bm㳿¾Ã!¨FZ­?‰R Ð‰^¨AGNbllGB6 J0303+0554?ïþ¦©8ÿ? Ä¥"¡pg?%•lpY? Ä¥"¡oþ?ïþfåO}?HÐW@Û…?)Ÿ'«"Š?HÐW@Û"?ïèSá¼Ú{?p&¼x»"?g¬C%†j?p&¼x»{?ïõˆ§ø¼Ÿ?RÃ^g#?Tî°†Àd?RÃ^g+4FGL J0303.4-2407?áOòÉU"ßÀNŠ›ÏÔ¿À7¤¿Ä¦ŽÀ;'­¯Ñƒ@g½ml
?ý"«þöë"?•p³W–ûì? w›ºR™@<ï>çœ\@š'ျ¿¿u š"¿×ö‹ÂÁ[*¿ß
X^©¿Üª½"µ·‡¿à·4µs¿Ýìðƒ¶-yAGNBLL3FGL J0303.4-2407PKS 0301-243?ïþr
M²?$ãb"??(ß+&ôí³?$ãb" ?ïý7y‡$þ?Nˆ@Ùõä™?6D3ÆØë?Nˆ@Ùõäk?ïÑîAʾ?|û"ì?wß ðÔ?|û"ì?ïÿà ì>å¿—;€>ï_ãå>å¿—<,4FGL J0303.4-5232¿ã3#¸G
ÀKVx|é_«À:NÇw"vMÀ<mÏt@3ÏDvQ–@Ð"<jêZ?ÄE¡Iç*?ËЗ;ÊÜ@c±€@,@@rwÅç«¿â\^¿âⴕžbV¿ëf¿§ C¿é©Ì·ÔD¿ïþÒ8F˜k¿ïð®SeâAGNbcuAT20G J030328-523433?ïüØ(θ?:j! ¥Ô?9>¹Š?Š?:j! ¥ì?ïý6ĸS?Q8[èoÎ?6OiÚ=_<?Q8[èoÍÿ?ï]W‰u"?'¡~क़Ã?4UÑMc?'¡~क़Ã?ïù"~vMt?>B9¼À?I²&Ê6Y?>B9¼ÀM4FGL J0303.6+4716?ìk-…x¶À#µx_.QÀ8rÆ	d,ÐÀ;˜äXڌ©@ˆƒÇ =@Ǧ†è½?¢§û\,PÁ?´Qç¾Àš@H<¯³·@Ԓ¾Þø?ޛà»íŸ¿ÜŸF¡úç¿âŸA¤:¿ã=OK—®¿æЎÞT´¿àíñ_©2êAGNbll3FGL J0303.6+47164C +47.08?ïø£²L4'?Jì1ây'?Mq6Ï-¸N?Jì1ây?ïêMÒn¿?€Z*ßÉ¿?e²-ó'B?€Z*ßÉ¿?ï‡PŸò?²èFgÇ
?Ž8«Øx>?²èFgÇ?ï¨ì˜ðŠ?n'•8ÃR½?…ÄÙüÃÝÎ?n'•8ÃR¸4FGL J0303.6-6211¿é—«OöœÇÀHYå\ËOÀ9Q³ø^KÀ<êg¹M@¨3vë@Ùb<5:?®É)¥?¸S´²ú"¯@c¤%
×@‰ˆ)"´¿ÞpGÛá½ ¿à6¹?|AÅ¿æªiËuµ¿äZTª|?ì¿ë(ÔɎտïþ²í'¶AGNfsrq3FGL J0303.7-6211PKS 0302-623?ïýˆ¿ºµ?/ÙµW·,?3º*aÌ?/ÙµW·Z?ïûՐÆË?\À$Éײ?@©¼äÓð1?\À$É׺?ï #WA?'ӏÌ
>?‡÷9ª/¹ä?'ӏÌ
C?ïþ^_Û´?sp^Scª?*D·AZ?sp^SeF4FGL J0304.4-2833¿ët¨'Ô©ÀNU<æÀ"À:øÕ!/$±À<˜5¤&»V@! pe˜¶?óV¡—"Ü›?ÙÃp,¸Å¯?ß(Ì|ðÁt@j¸A$@eK#É3?ï÷D9ë´?ï¢.(1wq¿å°'b"s?Ë´¯¼пݳÿ¡`bk¿çûûŽ7£AGNbll3FGL J0304.3-2836RBS 0385?ï潩XBT?n1À"(Ú?iBV§½«ˆ?n1À"(×?ïÐqú¥d¢?¬92	H͓?wÇ­M®\?¬92	H͓?ï nùB‡ü?'ðÁb·~?›ò ׯ_?'ðÁb·€?ïd·<‰ˆ·?‰Eâ#?"inÎèí?‰Eâ#4FGL J0304.5+3349?À¦—®áYÀ5\ÂÅâÍÀÀ:ˆÝÇÆӏÀ<ڀ¶–@ò1Xèy|@æΆ
pœ?Õ
å=‡?؞œã¦3@_¶™" ä@%#ûݱ¿ìºÁ5¿Õ?ëAµ!_v2¿ê»à¡¿éáìžú+«¿è²2·ã0¼¿ïéXü˜AGNbcu4C +33.06?ï"Oߘ!Ü?¢`^C&_Û?Šì÷ˆœ?¢`^C&_Û?îÜ0þ©ã?ÁÈ`¾c™)?¯B<ðaÏ?ÁÈ`¾c™)?ëÅ·8¿'Ì?§'*Ê©í?Àé#¸Ó?§'*Ê©í?í–t"¿
D?¡W¦›-X®?³L[Ú•Ù?¡W¦›-X®4FGL J0304.5+6821¿î!-rµ_~@!.Ÿê$ÌÀ8Í~¼ž`À;SàGÓÔ@^^ߎš@[\|ؘ³?°­xH¼?ËK­h¿@U§L	ÃÎ@H®ÅzÉ¿Åçû;õún¿â½:ZMS¿èXžâ¿éÄÜޒÇî¿ëyóa2¹¿ïþú¡Ç:'AGNbcu3FGL J0304.9+6817TXS 0259+681?êbyŠ¸x?ĝ¡ñ´¢?ÆvµÕ?ĝ¡ñ´¢?å6jØe?Õ»ÑL`?Õۓ*O5Ý?Õ»ÑL`?å‹ O"­,?¸*5èHÁú?Ôé¿`Ö¥¦?¸*5èHÁú?ãíÇF.{€?µÀ¬$›ÃP?Ø$qs£	?µÀ¬$›ÃP4FGL J0304.5-0054¿ïßAº.¨ÀHXǟfb5À:â,[ØÀ<žBuÆ@Ì0ÐWpÕ@X϶¤l?Â.ú(ûvÙ?€åƒõ9õ¼?ÀqU­±~"@³>†MŒ¿ïû–ÿ‹eú?ït¦Àž–.¿à(é}Ý{q¿å
*Ž:Á¿Ü"±þ?`"¿Ê¦2™°?ÎAGNbllRX J0304.5-0054?ïýbÊ2Oõ?2þUïâa?4é®m€P<?2þUïâh?ïþ]‡Š@?Dzˊƒ4¹?*'Ž·\	Ï?Dzˊƒ4Ç?ïҋ£¦_<?yßÉކ
°?vº.,Ða˜?yßÉކ
¨?ïú,¦¤|?;Rî•\M
?GMen
»€?;Rî•\M4FGL J0304.9-0606¿ï¯K½FÜÀIû5ü;OaÀ:´BˆCÀ<|vOèu @Þä^9@æCåÍ?ÊÅ4'$E?¬nÊcª?à52F¤)@@â)é•ö¿âÄâˆô'¿ÝG­¾"¥¿¿â$ýh %¿äL<ÿÂ«¿ã_iG¿ïÿþó…õAGNbll1FGL J0305.0-0601PMN J0304-0608?ïþëáӅI?µ=½^Ü#?!AâÇ«l(?µ=½^Ü|?ïþA¡'ë?L0O²)*?+åæïÁT(?L0O²)B?ïމå@ñN?r§œr™è±?p»
_‡Y9?r§œr™è«?ïüš™yÜÞ?,¹lø=?;+41A?,¹løg4FGL J0305.1-1608?èoŒ·/cÀL•!Ý Y§À:€'_ét£À<k7…¨K@!	‰Í?û€N¤¨ÁU?ªÄw=Ï?®. |wJ?îÚ³	­'ì@
þ"™Or?ïÆÛl6Š¿çµÞÿT^|¿×ÐPåË¡T¿à"H÷À–¿».ù<ÂS!¿à.ŽˆÄ_AGNbll3FGL J0305.2-1607PKS 0302-16?ïÿˆ…Ïû™?#ÞïÒÇ?
ތ̌?#ÞïÖ
?ïþ¥Ç%??
Ç"Šû¢?%£ý®¶›??
Ç"Šû¼?ïû+,(Ô?Dä¬t"xp?CSO]ø²Õ?Dä¬t"x€?ïþgæ}±;?•‹o¼§x?)˜$ìBÉ?•‹o¼¨4FGL J0307.4+4915?ïú±"ÀGc€X€À9
¾.¤XÀ;ªQ­q½²@µ$h?ÿ	GŒ†‹ ?­Nçï'õ?¸ Š6Nœ@©ÊAR@ãTpšœÏ¿ánoês¦Á¿ÝÃT~–¿Ù3$º¼)¿âÎg öo³¿ß6#¨{µ¿åû¦Ôë?AGNbll3FGL J0307.3+4916GB6 J0307+4915?ïñÎàh€?\׽ǘ8\?\üb?/t?\׽ǘ8R?ïMnùeW-?°äîMT?–R ÓU[?°äîMT?ï>-¦?˜?"œyLê—[?˜?K8Þ?"œyLê—^?î4÷S"}?"?Ák*"?¬¾`ŠÆÈ@?"?Ák*!4FGL J0307.8-0419¿Ç6€
o¿ÀI%ŽÉ[ÿÀ;`ØÞ¨—À<°yixiž@ÆðŒÅuÀ@ڒ_ét£?Î'
)¤"?xÔ â«^Ó?¨D<ߞ$ˆ@åGÂâ=?ì©ðÿ±üg?îâBµ‡5ê¿Ý‹@»\¿Õp^aàÜ¿é'Àoz¿´ŸEÀ~ŠÊAGNbcuLEDA 095522?ïðô ò'Q?WñfMpª?^¾Ýb?WñfMpª?ïü¶PÏ?Yú6ˆ-?:Ky‡9¼?Yú6ˆ:?ïœkö¿˜0?†qÞ4ea?ˆåPóž?†qÞ4e\?ïñ‹ybº?P	R$ò?\é
é:Š ?P	R$ï4FGL J0308.1-2852¿Ðú	Äm
µÀMðX>…vÍÀ;`Á¥À<ĦÚ'Q@À$¢ö@_ƒôç?É秄ô¤?´ßª_‡?èC ´@ZÖ¼å¤?ïãq¿_üÀ¿ã0
¿0W¿Øò@#Ü~¿æH¿AHõ'¿Ö
HÞI"¿ïÿ·Û¤%AGNbcu3FGL J0308.4-28522MASS J03081686-2851054?ïÿr ÞPa?ùT_ÂÛ¨?«ä5óú?ùT_Âۊ?ïýÞ'3WÔ?MËÙô.Ò?1ÆeAY*?MËÙô.Ò?ïå	¸''?qŠ0Fõ¢?jöGm}}þ?qŠ0Fõ¥?ïû#Nªç?3Üá.rÍ?CrÅÉTh€?3Üá.rË4FGL J0308.4+0407?Þ[í!¿
8ÀF@ûüe@ÌÀ9r×;»—ñÀ<K]Ìcñ@7žÐP?þ"°hè÷¦?²rÐWîï?³»ÀNÓç@Ôþ¢1î@
(Kù}°¿ïkL"=?ïôµ^œ£¿à}Ôvå9«¿ÛÊ÷_tp¿ã¸ÅÿS1Ö¿ÝI‡Þ[?—AGNrdg3FGL J0308.6+0408NGC 1218?ïþ€#¿ï]?$£qJMe¹?'ýÄ
$?$£qJMeÏ?ïý;&ùè?[ú€ði­?7ö&È0Ə?[ú€ði³?ïÞË>@¾?s#ž¶^$?pš`ô_ ý?s#ž¶^$?ïî7A4ë?VŒ[K?arȾËù?VŒ[P4FGL J0309.0+1029?ìwôÐї¡ÀCÛ×Ûô‡ýÀ8ÜG©â¼ùÀ;¬éïóB'@e'æèW@Îy$¯ò?©çØýî¾ö?½Zç,IŠ
@´'\e[¤@ÕH©0տ؏ØÛMîö¿ÜUÝað_ú¿äEÂÖ[¿ç(àwúc¿çH©©µ¿æE»ãAGNfsrq3FGL J0309.0+1029PKS 0306+102?ïý´'.ˆÞ?1ÎU}×Jú?2[
Ì?1ÎU}×Jþ?ïùÚÝ{@
?eÏÝ QÔ?H"Šÿ×?eÏÝ Q×?ïŸ"}vfË?† ‹7(¹?ˆ7`¢fLó?† ‹7(¸?ïÿ³bö>ø¦ì.I÷ç?§'ßR>ø¦ì.Iø44FGL J0309.4-4000?Û£$8®$ÀM`_ö"FÀ;[­÷õoƒÀ<ÛÑ_ÄÖ@ ¤{jÚin?ûæ ÆI%
?ËÁ>â=ø?¼(ÝÄÁ»w?óܨ##ñ@ïkY?aj¿ï€x–Ó?ïý Ê]¿ÛD!=<v¿Øtâ*,#t¿åjÛuÜûï?³¦G":AGNbcuPKS 0307-402?ïþô	p?†‰dA;a? ·/oÈçê?†‰dA;?ïùË='(e?a³Þ2þž?HÓ	»^h?a³Þ2þž!?ïï"foá¨?d	ˆNúL'?`ݙXô?d	ˆNúL?ïæ±N°í?]û7iÚ­ã?iúN±O?]û7iÚ­â4FGL J0309.7-0745?îm&|^ÉÀIükßL+RÀ:`ۋ¬q
À<b//˜t@Çñ²µI?ýï¥Å!á?ċ–€_Œ?·›ùñ9!?ñÀ£"î^î@Oá>Ê?îÂWþė¿ãW²8ÌÐ(¿ßT|Yó¿Ç˜iwÿk¿ë˜š`höd¿ U8»]dAGNbll3FGL J0309.5-0749NVSS J030943-074427?ïñÎ{uš?[tƒrµM´?\c	Ë¿?[tƒrµMª?ï÷NÀ?fôcMdŒ?Qb~"Ö߀?fôcMd‹?ïR'Y‡'Q?"1ètróD?•­ÔÏ
ÕÞ?"1ètróG?ïÌ<WtÚÜ?ll:"Þµ?yáÔE''e?ll:"Þº4FGL J0309.9-6058¿³ÞaÀ²'xÀHxj¹¦À8c9‰Ž‰›À;á"0ÉÌg@ýØ@N°œë]²?ŸŠz¨ùÅ?¹+
÷fÿ@‡¹E @¥K#É3¿¬Õ²_ÊQ.¿ãP;å‰\¿ç1tØÂú¿çÖÆz£¿é¹…\˲ñ¿ïïÉQIÉAGNfsrq3FGL J0309.9-6057PKS 0308-611?ïû×l<þ?<V$vVª?@£'Or?<V$vV·?ïö‡"5?püÌø'V7?SÀðוà'?püÌø'V:?ﰘÕ}bÕ?…m¢eCsa?ƒÙÊ §J"?…m¢eCsi?ïþ)ì9?#™Ž"ÄÒ?.Ía<sš?#™Ž"Äz4FGL J0310.6-5017?îæÜ@÷>ÀKmÖ¾¾QÀ:*Vˆ¢ÑQÀ<a€OE¸q@ yޓô"?üs$ºÊl?·•`ÏΉæ?©A|÷øI¨?òª—ƒ>äA@%"z£Š3¿à=¢wŽ­?î½:¾AÓuNÌí¨¿â©?ÿÊP¿¬yšÜËٙ¿çÝúºpªAGNbll3FGL J0310.4-50151RXS J031036.0-501615?ïþû¶—êÕ?b+'9¯>? D–R´N?b+'9¯?ïþ
èÿýL?I'Ùé?/!p+?£?I'Ùé?ïã;·ˆÒ?syãåtï6?lÄàHw/"?syãåtï@?ïý"E?4?)9SOêà?3Ý×æd1?)9SOê²4FGL J0310.8-1041¿¿ LÐäðåÀJ¬7'MLºÀ:þˆ†KÞüÀ<‡]°µ?@ 8ä¥Üs?ÿë¯æâøˆ?Ç-fe§?ž¯×žŒón?؆|¥@¶…8?í¤.}ÁÌ¿¿é2þ'W¿ÅÞo¡ùd…¿è¯Þ|¸¿ÒÔó"õH¿Â.åE¿|ØAGNbcuPMN J0310-1037?ïþH5.ã?&¨I$Qš?+|­Èv?&¨I$Q;?ïý£"a?Nžóo<˲?2æï÷Y?Nžóo<˓?ïí$Ñ΀Ð?f*¶¯ó6?bÛ.10ã?f*¶¯ó?ïü<My÷Ì?0´Mׁ?>"0A¦`?0´M×s4FGL J0310.9-3458¿åþV\ÀM¤N¤¨ÁUÀ;cârPÀ<æTe²â@@D[GNs+?ýÆ,Ÿ›;Z?Õ:ý Ë?ÀáŸlÂK?é9¯ž¾œˆ?ù-‰Ó¨ß?ïüà[
‡¿â˜¹Z)A¿â‹Y?aiÒ¿Òɧ~^«¿ëÒ/]•?Ջ÷-âAGNbcuGALEXASC J031057.27-350033.4?ïû'øi‹?IßuÁ¡õË?A¸²YÓ]?IßuÁ¡õÇ?ïâßo€?|μÙll?mæp ~å?|μÙlm?Ò?‡×?=ƒ?‰R>‹|z0?‡×?=ƒ?ï¹¥3m‹©?oÎë³r&?–³$…?oÎë³r(4FGL J0310.9+3815?ïÂÿ•Òï¬À0ëã}é9ëÀ:
ZÊPñŠÀ<:"^žñÈ@0z·\Ç@qg#$È6?¿íQ҅že?¹Ç}W™™ï?øÒÅjüZ@äl$ko:?ïà«ÁºJ¿ç4éKˆ"¿ã â-‡!È¿á³/'N¤S¿ío
D& ~¿ï×ó;Ì^éAGNfsrq3FGL J0310.8+3814B3 0307+380?ïcÛ?_˜ÀHKä?`p]œí%n?_˜ÀHKÙ?ïîÆñ_ñ?zkÙÊÚ}ê?a9ù B?zkÙÊÚ}ì?ï}'dÅ?Ž—ÉöEÎx?O¿sg]Ô?Ž—ÉöEÎ~?ïnx»¯%?|›ž("'?'?ÐèŠc?|›ž("ƒ4FGL J0311.2+6856¿ïË1½.–@"͒·þ¯À:¿ޱџÀ<2$fÖ@ ¯ø
é(?û‰Uê`o?ÒEÇ_zŽç?ѝbœ,p÷?û-%g˜•Ž@ æõ—ò%¿ÉÞºu‡@§?ë­ÃAޜ®¿âò¡r«ï¿Ùˆ›dÊÚÚ¿æ$ü=s¿Þ"˜±<MŽAGNbcuNVSS J031111+685610?ïÞWùûz?q¤G'îþ?pÔrÃf?q¤G'îü?ïô+ÆÙÿw?p2õ5Âù?W¨rL¡?p2õ5Â÷?ï¥M!ßW?–Gšß|+¶?žV[Ä=?–Gšß|+¶?ïlAÅÙŽ?iPs~Æ?'wÇDÝÎ??iPs~Å4FGL J0311.5-4402¿×{ŒToK)ÀLž¡3ßÀ;e'Ýãu†À<ãñx7@YvT3ˆ@pµ'-lJ?Âϼ<0Þ¿©in"?åkÛ@#œ@,¶ùPäI?ëËw͖÷(?í+¡~•\H¿ãÝløPß¿ïÿ ÿ¿h`?ïý''N#z¿à¶Y"±ðAGNbcuGALEXASC J031103.24-440227.8?ïý"ä;t?=哄o×?3`Þ$[,?=哄oÃ?ïþzÛ¬?C…%üK®ƒ?(^þrE:?C…%üK®?ï¤É¿ø"?…¶±${Q8?†ÍÏ[z?…¶±${Q5?ïÿŒ¦"&‰?¶Vs)ì3?ÖZö]©›?¶Vs)ë¦4FGL J0311.6+4134¿õ.&	"À,ô{gkÀ;z/—@À< !úü‹@!mˆô…Î?úO}¶åû?ÙFf@Ѭ[?Õ,ÅÛÁÝ0?ùoz^Ù@g"#ìÞ¿Ñ5®ÃLpq¿çæf0¶1¿ìNÚX¦ŠC?º#Rë__¿èe;ÞÓ_Ž¿µ 8š%Z­AGNbcuB3 0308+413?ïù¼r3?QïÞ·¢m?Iâ73åY?QïÞ·¢d?ïþ6'#?H2Iñ0?.ŒŸFÝ×
?H2Iñ ?ï©Å	]ú€?"Ç"Y÷*#?…Ž½¨_½?"Ç"Y÷*$?ïîÕ¥‡?Xi˯!øí?a*áZxb‹?Xi˯!ù4FGL J0312.4-3221?הª˜4ô"ÀM‹ºÜ	€²À;ylÛM™À<÷#a	/@Þóú?üã¥Áƍ?ÛæŸê$Ì?Ñä"''?úNãx	üÙ@ía½ª?ï±ÊÛ[¿Ñü×V"ŠŒ¿å¡@Aº¿Ì!8	ã¿è)Âbæ¿ðAGNbcuNVSS J031234-322315?ïûՙ"?FK²8¾
*?Càñ©™°?FK²8¾
$?ïùÁ¦#ò?b
«['c5?Kèùgp:Ï?b
«['c1?ïm(¡+È?Œ¥gÎIʖ?'Zýkچó?Œ¥gÎIʒ?ïÓÐ!×\?d€aRË°#?vïxÒ~?d€aRË°4FGL J0312.5-2221?Ð?	)2ë/ÀLÛƒjƒ,À:8†-¬
µÀ<bãv\}¯@ N™@-m?ú®4Ʊ)Ù?Àtv‰õÛ?ÅF×)òíž@I¢ÿsé@Üwý½…‡?ïÿì´É È¿Ýq ~¥¢f¿°¸'Ï&ï-¿×⛠}.¿ÜXJy¡¿ìy&\‹RAGNbll3FGL J0312.7-2222NVSS J031235-222118?ïöòpæ?R·(£.Ã?RÞ3Úç?R·(£.Â?ïøQƒhÂ?g ÈNë?N¹ò\÷‹?g ÈNê?ï}ZHš3Š?NµyCÉ?T¶ì¹Žª?NµyCÊ?ï¢ì"UI¬?rR'—g?‡D÷j­"±?rR'—g4FGL J0312.8+0134¿ët³¥œúÀF½ke©¨À9ƺNEqÀ<(ó"Çz}@‹‹«sÄ@-òˆH?ºùµkŒ&?¶U¶ë¹÷Þ?ù˚¥—Õ@»I)"£æ?ï͐â:ó¿Ñ!DÚ$¤¿åMú>ŸøÙ¿ããe€À¿äéëÁ"š¿ðAGNfsrq3FGL J0312.7+0133PKS 0310+013?ïþ
2ý<?.mó	k5­?/_Ð,Q0?.mó	k5?ïþ4¢L"Ì?Dl®·¯Ñ,?,µÛ6³Bâ?Dl®·¯Ñ.?ï¹I¦ß?€ÏɧÓ^?¹mº–HI?€ÏɧÓ^—?ïý•t7ÜO?$g"I'ž?3T^A‡¿?$g"I'34FGL J0312.9+3614¿¥'Ù•PŠÀ2i¶°_¯À:ieõ'_À<?
 ë2@ žôÄ7§â?ýYÞ7X\?¸Ã…¦G§ß?«I­âÀ˜Ñ?óÚE[Sã­@±(Íÿ|Í¿ïýgß?ïãϝ·‹r¿ÈqMàˆ–g¿Û±dÜ£"¿äeÜÓ«
¿ÃÏéŒÌAGNbll3FGL J0312.7+3613V Zw 326?ïöópdS_?Q'ÇþBY?R7Y?ñ?Q'ÇþBX?ï÷À¸7vä?jŒêïé@?P~':ƒ?jŒêïé@?ïÒ¹©aÉ?|Ô¸®«?v£+O?c?|Ô¸®«?ï'92ë>Ï?}ê]$xãö?q³E0KÏ?}ê]$xãö4FGL J0312.9+4119?՝qEŽïñÀ,7A¿½ð'À:7"¶
m§À;
ñû@§Ï"þ)f@+¹!]¹?»O'ÿƒð¿¿W4ð!»'@f"f\Uk@	¼óíx¿ØÔDRÈû¿Ëcòl¿Áj¢
Vp$¿é~0O‹Y¿ÅV1ûOÂ
¿ðAGNrdgB3 0309+411B?ïØ."ùò?"µp;CK?s轃ð·?"µp;CL?ïí†y4ˆv?.P¼þ=?by†ËwŠ?.P¼þ=?íElHšŸù?¥	DhQ/÷?µÔ»+;?¥	DhQ/ù?ïåæá^C@?aŸun¨[R?j¡¼À7?aŸun¨[P4FGL J0313.0+0229¿Àgì£+/²ÀFhfýe
À:×+•°À<1œñ<îž@•<F,_/?þŸ°i¿·;?ÜØÄ|Ç%ï?Þùà@ÇñF?ûë ªšrÝ@áão{ë?Ûh $ã1¿ì;P8&¸¿ÝdgE‹%¿èIŽ;Tj¿ïÿÌÔY‰¿ïÿþÐñAGNbcuTXS 0310+022?ïüšmÓÕ?C±"ÛÎh5?;,—ùaMd?C±"ÛÎhA?ïü0'Ví9?T9¹œ<3?>{uH–3Ç?T9¹œ<,?î<¡
…Y!?›ôêèFn³?¬5ïWªmó?›ôêèFn³?ïٟkú#9?bÝ|®Ã?s0Jîcñ?bÝ|®Ì4FGL J0314.3+0620¿Êì+Fx¨ÀDñLìAÝÀ:\¶wòÀ<:Š:N@ Ώՠ…ò?ün 9[ka?Ɩœúw*?½[$À?ôdõgö‰_?÷Տ;qÆ¿±§Ð(Q¿ê^ǀ݋¿Ø oA{P¿ÉWX×\»¿äíÑÅZ¿Õê€Ý
1²AGNbllNVSS J031423+061955?ïú†wœÁÔ?AYBáޅÏ?Eæ!Œø°ï?AYBáޅâ?ïÊD?çi?‹¨r—bÊ?zòÝàKP?‹¨r—bÊ?ïã·]wy¼?s>ù6›?lH¢ˆ†B?s>ù6¡?îΓgÃï??‹	Š^W$ß?£ɃÁ?‹	Š^W$ß4FGL J0314.3-5103?í=÷à1zÌÀJü©iuÍÀ9¨²ã»-À<XKƒÂ@úñw§Š@u_þmY?°S	<i½´?¤-?SR'?õ²`Š"Rà@ˆýµLþ`?ïè'á´,¿â±Ÿµ<O¿âtô3C#k¿Ý¸ãÁ…ñÇ¿âÖÑ"qïÜ¿Þû:]ôÒÐAGNbll3FGL J0314.3-5103PMN J0314-5104?ïþÄkJ6ö? aA}›Ï€?#¹K\¢I? aA}›Ïp?ïýÄúΦ?KgÐn·f(?1Ø)ŠÏŽº?KgÐn·f+?ïöX/n˜?bvØ6·?SO¡#úÒ)?bvØ6¹?ï÷ñ·-CÔ?>\1ÛE'?P'¥xZÏ?>\1ÛEB4FGL J0314.6-6549?ï
?§&øaÀF¯mÚÎîÀ:ʘòª¬çÀ<¡öé	:@1ª‰€ò¯@')Àê?¾"ÛÍÐf¿—àõ@?ƒ?ÕÇ,#õR¨?üêõçÎ/ù?í™ö`ÄæÏ¿æÞÕþ¤¶-¿æ·é{Y<²¿åK¢•ÁÅ¿Úaf'–¿ïþÊ-ëÌAGNfsrqPKS 0313-660?ï÷Ô26?Nñ$:…[??PW›"õÕÌ?Nñ$:…[F?ïàl—ú?aîó`}?o"ìhûÊ?aîó`}?ï¶9¿ˆn?zwŸfêñ?'qÿ$·?zwŸfêå?ïę 8Ñ?kyœŝ€?}³uoã—?kyœŝ~4FGL J0315.4-2643?èCÖCïvÿÀMYÝÁç–À;M¶Šk(À<¼½qåöi@!
K^"E?ú¢Ë;Óå?Él'Ê !É?Ǎè5ˆøâ?þD*Lä'@žq-êžð¿ïû—?ø¡¿ÝùV-3>ò?ïùÄýuŒ¿áaÏ}×Z¿àž+ϑ£+¿ãåªê#õ©AGNbcuNVSS J031527-264400?ï÷'<?IBDÚ#ÄS?P ì˜ÛŠ?IBDÚ#Ä^?ï÷ÊiW•E?fÄى'x×?Pk-PÕv%?fÄى'xÐ??…KÝAª9?ˆúú?;þ?…KÝAª5?ïÊƶt–ë?oª¬Ÿ?zœ¤Å´‹b?oª¬—4FGL J0315.5+4231?»"Ǔ¨o‡À)¨Ût´À;lŠŸ*ÓÀ<—!Áçã@!rg‹T‡l?ôû…—"¤?ÜýŸ—Šv?Ý×(›T¯°?ø›ÌyÁ@A:¤Ék¿à>ÀÕó'¿å*øf®ŠÂ¿ê­Ù!nå'?µuc.xŽ\¿ãâÌ'ª¿äµðè5AGNbcuNVSS J031527+423249?ïú¯–Apn?Llh6øS?EA¦ú>H›?Llh6øQ?ïýt£P~?`–é2°ã?4Zç|Ã?`–é2°ã?ï¹ß å2'?€ôËÅÉgÇ?ˆ7Ƴ[Ð?€ôËÅÉgÏ?ïöq)ÂÀƒ?L	Â=Sž?S¬z~ûë?L	Â=S‰4FGL J0315.9-1033?æOÔ/^ÙÀJŒCoÁYÀ9‰ÞNÕP)À<8€eëí$@#Pn'i§@tpë$¦¨?± $"I+?µÈNŸ¥m@uûdÌ'@CîÅ&?°È`VìÕ¿á9äþú2¿è𯮯¿äŒ <Àü¿é/–Ð<¿ïñneZÎAGNfsrq3FGL J0315.5-1026PKS 0313-107?ïüþ'0î
?3'ôVY(.?8Æxšw?3'ôVY(/?ïþF·ªaN?Gi®5ƒs?+"…Yë#/?Gi®5ƒs?ïÕÆx1ó?s‰YgQ?uöCç?s‰YgU?ïþ¥Ë['ý?¹ÓºK;?%£JGÐ?­?¹ÓºKÌ4FGL J0316.0-5626?ŸeC§"ÎÀI€Ç`|À;"¶Ò"mÀ=½‹ç)@ .ð%ä?õe¯ò¡r¬?ä=n q¥	?ä:ß%"å@÷üü?@•Æ1}%›¿â"ií£ù¿áß
váí¿ã‰Â@׶‹¿Êùá'çQ¿â©9êÝY¿ïÿÿ&¦³AGNbcu1RXS J031613.4-562545?ïõȼtO?TaøÓz?Tn‡aё?TaøÓw?ïýdv–m?NQc…Ì=?4ÜKL—á¹?NQc…Ì<÷?ïHÁ;l?‹O´Ü±?ç؝rl?‹O´Ü±Ž?ïé5tÉó?]êlO@4?fʋ<v£?]êlO@3÷4FGL J0316.2-6437?×ìêZò™ÀG|"µÜÆÀ9êHX^eçÀ<3Ð&ô`@fyɹå?ùpÃLŠÆ?·N[ؘÝÝ?½û&Qxm¥@	›ü"$íö@ƒýLŒx¿ÒLŽ£ò8¿£‰9¥H­¿®·}bßÑÀ¿ÒŠ4¸Œ¤¿áqÊi¿×ÙFWÓ%¬AGNbll3FGL J0316.2-6436SUMSS J031614-643732?ïޓÄIÓÏ?q&®v£·?p¶Ûß?q&®v£µ?ïô‡Ú,Ü?nY¾IŠã?VðK˦GÏ?nY¾IŠê?ï‰ßù"¶,?Šísšc•Ÿ?ˆ·Rt¤?Šísšc•™?呂¸héf?pPÃ3$ù?†_ÑåŦ+?pPÃ3$ù4FGL J0316.2+0905¿è¤viŸÜÀCɤi×4/À8¹g«
fÀ;«ÇQbÉ@®Ô²?ýЕÊ@r?©`¢G'Ý?®õ|æ§â@¸G¢'v@9Äè§É³?ïöæç*F%¿ÙÐwœn¶¿Ý©·ôÎs–¿ÚCyÒSõK¿àðíޕL-¿àí¯e³¹AGNbll3FGL J0316.1+0904GB6 J0316+0904?ïþ?ëx?%Æ®4šØ?,H~þÝ}?%Æ®4š×Ü?ïýc±_ü»?PÑ,`ï—?4âuÿ?PÑ,`ï?ïØÓ?Žx?yû×z†X?s–`8úDN?yû×z†Q?ïï_çwî?N¬Ô÷; ,?` âˆá?N¬Ô÷; 74FGL J0316.2-2608?îYώZÉ!ÀLݍ%íÐSÀ9ÇøåY‹À<6@<H†@…[f=r?ücZ'ó+?µ\ÿ	Šî?¹s 
Ìã@Ì|Dôü—@PhÖ-H¹?Úöóý=Wú?Ïk>¬¿áŒY	†'¿Ð娶m¿äÕ\Rç-¡¿Ù›2Ál"AGNbll3FGL J0316.1-2611RBS 0405?ïä\¿Ž-?f'ÞŠ?kæ£@qÓ?f'Þ'?ïÃr¦<ÔÒ?™¼ µ¦c?~F¬á•—g?™¼ µ¦c?ï~úó.Ld?Šam,Âü? ¡š6sˆ?Šam,Â÷?îð>J¥L‰?Œ¡'{ô? üU«7l?Œ¡'{ò4FGL J0316.8+4120?ê]X,¶ñÇÀ+g0«¼²À:z®Žd•À<	›h¦²‡@"YBI-Æ?ý[8jª˜Å?È=º ¥Q‰?¾ú|2€†@Pÿ}¤§?ç:V[Vh¿íœý
y¿ÙBW}ë=P¿åqÏ ¼£Š¿ØÑN;Í5¨¿Ð¸
ãmx)AGNRDG3FGL J0316.6+4119IC 310?ïþôõ\Ot?ó6PcmK? °ª;¶8?ó6PclH?ïþlI©\é?ESµ/ÆAœ?);ej1mÇ?ESµ/ÆA¡?ïæXSá§?sO?íâp?i§¬Xâý?sO?íâm?ïøRfÄ6Ð?CüeÒtÜ?N¶dï$¿¯?CüeÒt¯4FGL J0316.9-0625?ïSCu͇ÀHÞìAÝ"À;Ÿ†B¤ÀÀ<©ÓåjS@ "DðIÿ}?ü,?ùë	?ÑA ^Y҄?¿¬œU¶•Ô?íÞ½ý&1@aÒ"ø¿äEå½_¿ë5ßàл¿Ñ«±EX¿ÝÒéý	U"¿à»ùu¢CŒ¿×]cß#'AGNbcuPMN J0317-0623?ïÿJÿ¿'1?ä/ý®? 
¹î?ä/ý®›?ïþcËzæ‹?C]qeqÐ?)ÃHQ—Gß?C]qeqó?ïö÷S(?H?Xzjûا?RY¯qà?XzjûØÃ?ïù	é ?;Åh¢y?I‹ÇØ[ä?;Åh¢`4FGL J0317.7-2804¿ïS©Ý…uÀLÚ'¿aª?À;ü/çCÀ<Þè	i5N@A`[	ø@þãþA¹ß?Ótá¾ÌY
?§ÂIÇI?Êê›ê¬±¤@pM
ú¿y¿ã-Æèl¿Ý¢}ÃÐ#ï¿çòbo¶Ç¿áhœ|&¿å#ßYw¿ïÿÆߢèMAGNfsrqPKS 0315-282?ïþuºW®Ž?#ÌÁ™$¥?(¤Z…"?#ÌÁ™$n?ïýüéYn?L–¨ö
@Ñ?0µ4•h?L–¨ö
@·?ïÐÔÔT?{fºN?w•ñþ•Öh?{fºN?ïüÚVÎ ô?+âÈíõÕ$?9-IŽøc¨?+âÈíõÕ,4FGL J0317.8-4414¿¥Ò¯4ÔÀL´ûß	À;¡óQ›ÔÀ<ïq"§š@!wi¹'G?ýnvÖ 2¥?È0î	ˆiñ¿Ž/¹gP'?Ç?·e‡nI?ý\?r±£?ïø"à4ê¿à L jÓ¿ç3f"‰`¿Í›ÅÃď¿æ¢BŠ"?УßBÆ#AGNbcuPKS 0316-444?ïþmèó?$5³4`½?)!~PÎÙ?$5³4`½?ïò–ù(ž9?q{'Ÿ?í£?ZÒ
®ÃB?q{'Ÿ?í¤?ïí»Tº?nc£Ž¯÷?bÿDè«E‹?nc£Ž¯Ú?ïè£Ó
ÈÅ?Xý÷¨…?g\,õ7:M?Xý÷¨…#4FGL J0318.7+2135?ënZ‡lÙ.À=¢Ž£œQÛÀ9{¤ÆôFÀ<˳È	@ÐõØ´·'?ÿõ±]½Õ?´¨ÜW¯>q?°¥¿AÉÎì?û‹ÐÚè@	T¯ƒeД¿Ùs†Ž$¿Ùv€d¿â_Ïoº¿Ø|10É¿åE!ýÖ¯û¿ß
Ë |âªAGNbll3FGL J0318.7+2134MG3 J031849+2135?ïý5Î6?/žŠù~?7~QŽOFŸ?/žŠù~8?ïý/©}³æ?Rˆž4Ò?6'´`ÒÈ?Rˆž4Ñ?ïò× ¥?a¯I+l¿?ZQð¾µÖÈ?a¯I+l?ïãVÅ)öD?ZÏÅ'ޖg?l©:Ö	¼#?ZÏÅ'ޖ_4FGL J0319.4-7045?³jÛ¾>DÂÀDÕa^¿¨øÀ;TÔ«¾_LÀ<㤢â¸@ ÐtcT8<?úW£öíô?ÏûÉ,9?ĺH¦7Û?÷Yn€ç-?ükà£Ä¿ççΰқC?âÞ¨—c^t¿Ô›½ ´ëۿ܌"aFA¿Îº…@q4¿épTü±–æAGNbcuMRSS 054-102986?ïøˆ[6»?Hûuދi¨?Mßâ"%*?Hûuދi"?ïúOó :¾?b÷øðH?FÀ1ž?b÷øðL?ïӚulp\?v~À^…?v2ÅIÇÒ5?v~À^?ïÃV©«ð?kZm"O?~T«wªÖ?kZm"O4FGL J0319.8+4130?ï@ÌÁ&hgÀ*" _ñØÀ5Ó²Jj‡À:H¡¸é@oÊ·sÊ'@_&DÉ^?"sÚ Ó}I?°œ}#Â'@'<-ðÔ@ ÷½1ø¿Ç>¢Q#¿ÚáÚ»wåÀ¿â#%¿,P@¿áe°ÿì·¿å`ð
j¿æE~ßÙïËAGNRDG3FGL J0319.8+4130NGC 1275?î± ©ö,:?§xYbH…†?¤åõ`<R?§xYbH…†?ïd}ÍÕ?®ÄœF ˜?"pFE_â?®ÄœF —?íDmN8jÄ?¨*íáç˜}?µÜ•Ž<©ß?¨*íáç˜}?ïÇßÍ4¹?zØÅÆ®Ž?|qe¢¤?zØÅÆ®Ž4FGL J0319.8+1845¿ÇV—&‹È˜À?²Ë…¤ðÀ9ârkWfïÀ<
øGv@!xH¥á%Ÿ?ùބ 
Q!?´½cù#ÂÓ?«³4uR't?øšc
»@;˜Í@åù¿ïöÇ¡Р¿–<¶áöL?ïÿÂWþė¿Û¢hu4¿Òܞ¼n/Þ¿Óg/x°kAGNbll3FGL J0319.8+18471E 0317.0+1835?ïÿÔ8?´8q@'?ß~™?´8q@Ý?ïýÑ1V(@?LÕìßÅfò?1vuN¾Õ?LÕìßÅfé?ïêiZL›?r7"ûuk?e–¥³bf
?r7"ûuk?ïþ—~? /®©9,Æ?(vˆQÔ? /®©9,¿4FGL J0319.9-3821¿ìtóË1F*ÀLˆ¦ YŸÀ:×ÜhKBôÀ<¤vtÑc5@JëêI_o@šތò?Ã0èU>v?¡"!ý=$?Ú'Òûº÷@	EBҍ?ïç/ï±Ô#¿â'eÀ¤"¿èÙà[DŸ¿é‹¾dª$¿Æ{ò>ÌC¿ïÿÿ" 5•AGNbcuNVSS J031957-381527?ïÿŽy³÷!?Àû¹·Y?a"7–Â?Àû¹·
Ã?ïþ×Ì3M?>[Yv¿]ì?"ƒ<Ë/9¢?>[Yv¿]ì?ïåq´¯³?k"Áµe?jŽKP~M?k"Áµe?ïþIpË?¸9‰÷?(oøóXâ?¸9‰·4FGL J0320.6+1125?À¢âÙØKÀB¤WÙÜÀ:·ŒR‰9ÐÀ<õ0™%@ Wò ò@… æ"ôï?Âó"`›2¿¥>" šœ?âhâý¹÷@2®Å$⸿Áe¶}ªû—?ì=ÙI²Ñy¿åç-É¿â(<县ⴜ>ån¿ÑXü…÷ü%AGNbcu1RXS J032037.9+112503?ïÀŽÄ¤+é?}pp€?¸­êõ?}ppÂ?ïðÆŽ'Ç?t%«-`˜?^sÂâÜr?t%«-`›?ï¦ob	öÛ?ƒúÙw䤒?†d'}'I?ƒúÙw䤕?勇׬¡?u:©Sd"©?…'JߗÒ?u:©Sd"¥4FGL J0321.3+0425¿¿š`XPs?ÀDÿ†ã´oßÀ:§S³ÜÀ</ý ª/@,ÂìÏ º@!_Ìr?Á4ˆó¯¿ª3j¾9?ê‹ÀBzÎÓ@äÉ?ìºåC¼s¿ç±à¸<¿æÏu¹Nk¿á|øCsW¿é&È÷U6"¿Î÷_]ÂíAGNbcuNVSS J032130+042628?ïÚø¿öý?oþIYÃE?rƒ vV?oþIYÃE?ïõwPv?k'ŒÓyC?UÙç_¯?k'ŒÓyBù?憎^GØ?ƒá¢B4õ?…]¨n	ú ?ƒá¢B4ò?ïä­þè¢È?V Ä—uÌ?kR]7Ô?V Ä—uÒ4FGL J0321.3-1612¿ãë–Ñ¢ÕóÀJÕf@¦¹=À;p%FáeáÀ<Ä#G,å;@/ëîÑ?ý橝ÛÙ?ܪ'zÁg>?ÔֆŸkë‹?ýÕ½6VÔ"?úBöt»ê?ëw¥ˆ»%?ï°iŠU_¿áj¿ÜÌú61ë¿ä,HÐ(¿ïù"O¶!AGNbllPMN J0321-1612?ï˘$M%?y¹<*'#?z3ðmÙm8?y¹<*'$?ïzØKi!g?ŸÝÎ4€R?¤ö'ÛÓ3?ŸÝÎ4€R?ïÎà"â?"ÈsÓ=L?œF#û¼ƒ¹?"ÈsÓ=L?ìÏv,|@¾?¥Ùê_õÝ?¹"Nœú?¥Ùê_õÝ4FGL J0322.0+2335?ÒöÄKoK+À;˜§'h˜À8ßaúÆÛÀ;М·[K€@^æÀ=ó?ÿƒëaãIç?§uëƒ`?‹~Ö¨KkÂ?ãYA¥Ã@øù²%?ïô5â:\¿àñ¦ é4¿âúúÁ»¿Û'ýûÉ¿àÃhjL¤ô¿Ùº å¾5ZAGNbll3FGL J0322.0+2335MG3 J032201+2336?ïûÚì!‰}?8G"ª¶=¨?@"OyÚ6?8G"ª¶=Ñ?ïûiç§ë/?b4»AE"?BXa`SBÒ?b4»AE?ïç£äwg-?t"¹Î?h\ˆ˜ÒÃ?t"¹Ç?ïÕÕæ̪?cÉ&ŽI¾?u™ªü0?cÉ&ŽI¸4FGL J0322.4+6606?æ<s
@Teè'%1À:%½›¡æÀ;¥KJ-'@Ri|ñBM@TÓ¥¸?Í%ÑuÓì§?Â(ÅÆôÄ?÷¡w´l"@mËÑ¥#»?ïƒß=g¿'¿ÌŠ|ºe¿ç
@/p¿ê¬t½—$ʿ竊\å´$¿ïòªa½à AGNbcuLQAC 050+066?ïçKÂ@T?l‹Ü*ìW÷?h´ÿ=¿¬¬?l‹Ü*ìWû?ï÷)þ?m")Ó7?Q­éôÄ×?m")Ó4?î1Çxe?¡r¶ÒDd?¬ãˆŽ©¥?¡r¶ÒDd
?ïÌÑ¡2_.?c‰9xºÛj?y—/fÐh€?c‰9xºÛe4FGL J0322.6-3712e?ÅùITCÀLX±mÀ9ÍàöO}À<Oʪ³Q@ÇìÀ24±@9‹q¸ª?²ðìçŸ?¨)>'·Ó?ö U?Íui@¨ÕzÆDÈ?ïZeÁû¸s¿´åcË+¿â³KQ7*9¿âÇÿÞr¿¿á>ÀÚü¿ÝŸœèÙrÍAGNRDG3FGL J0322.5-3721Fornax A?ïëËL"Ë?`ËSè«ÃT?d4÷³{4B?`ËSè«ÃU?ïûùÖïÜ?TÖT›äƒ>?@¤Aˆ™F?TÖT›äƒ@?ï·jRE'?"чm¶?'%}ën›Õ?"чm¶?ニzã)?hêo	Õ–?€^aO5Â?hêo	Õ›4FGL J0322.9+0940¿î@gŒÞ6ÀCŠ'¥aNÀ:ËW´ûßÀ<$ý~E€=@òÁ	J+@1fàé´?ƑཚÉ¿_Œ‹Û?¸*žd.©?ÿ›£4"¿î
ÍHÏD?ÌfH'ZŽ¿æs½œ®!¿äYQªí¿á.¯½µƒ¿áìà¾q?]AGNbcuMG1 J032256+0941?ïÝU"qÕ?p9-#€ìú?qUnÇ~?p9-#€ìø?ïñ'7¢ñ?t×^ÇDþÈ?\ېºÃË?t×^ÇDþÈ?ï{3÷@ö?Œ,•ˆoÑÒ?™á<ò?Œ,•ˆoÑÇ?ïÛL¦1'û?cãaï£5©?rY¬ç6²?cãaï£5±4FGL J0323.7-0111¿Ï»×ìG
ÀFœÙ¾L×IÀ9y|"MÀÀ<ýð[GN@²S~'<?üöñý2Æ?³†þ6|>?¹ œ,ÆÝu@ª`%څ@ã‰û÷Þ?ïÿ-<y-¿ÅƒÙ¾Í±¿ßúTvyÚ¿ÑyzϪ¿å†Ö]ð 9¿Õ•:¤Á•âAGNbll3FGL J0323.6-01091RXS J032342.6-011131?ïóÓ¦é³Ñ?SÆ=@¾Ä?XX²,˜\S?SÆ=@¾Â?ïWQµþº°?¯þH¤ú_à?•É@(©ê?¯þH¤ú_à?ïn.~c¤?Žò-'/?':?3‹}?Žò-'(?íèwá¨XŒ?"	2YËÙÂ?°¼@ò½;š?"	2YËÙÃ4FGL J0324.3-1313¿¹ŸÝ=*|ÀIÙÕ<ÝÖàÀ:ƳÑSDKÀ<rºÇË)@¾Z.t²"@l'	Z?ÅÔú˜¸?¥CÃW®?àLS?È@f¢$'–H¿Ñ-!¡:wË¿æ<¿ß®Q¿ç/SàQäÏ¿ã§CÁð`¿êÖ
ˆ~¿#¿ïþašNË?AGNbcu3FGL J0324.5-1315NVSS J032430-131002?ïó
ûO4è?T*zñ3½?Yä	a–.¼?T*zñ3½?ïù9"¢?b@@a8?KóuwÍ?b@@a;?ïͪþæÙB?|ʸü?y*€Œ"_•?|ʸú?ïðx~rÔ	?Kôd
ÒLß?_Wñ±?Kôd
ÒLà4FGL J0324.8+3412?Ì7ôÞôáõÀ2¶®::ŽqÀ8­<Íè«À;±5WСn@—#ȇ@)@k*?¥ ‰ª
Z?­‡½Úy?ÿÉóÔx"@#ò‹ù
¿Ù뎃æÔá¿çöÌ ,/߿ꉢ«'â¿éSÐ↏¿îcó¯5?äÆ@–žAGNnlsy13FGL J0325.2+34101H 0323+342?ïþ±‹]²?#\g7¯(?$çO
$Ù?#\g7¯6?ïü¾Qìƒ?[²Vpa'`?:p›ÚÎ?[²Vpa'm?ï\L9Ìý?Ž×-ØGb?"vxÆ`_è?Ž×-ØGb?ïþÀå˜"?ú`ƒ¼s?#öñ¦vÒ?ú`ƒ¼r—4FGL J0324.8-2043¿ë™ó°ÏjÀÀK?™ÜµxÀ;hi²KAGÀ<ÈõZŠ@ "¤Ht8?鏂¿b€ÿ?ß>P}pï?îøÒpXƒ@i΀+3Š@	î…äÛâ>?ïùÈþáòÏ¿ïñ"ݝ)œ?ëÈòíÈÅ×?µnTœdz(¿åvpnö¿ïÿÿ" 5•AGNbcuNVSS J032451-204324?ïÿ"8ä%t?§›ª3z?ñÆö¢Àæ?§›ª3yâ?ïüux‰Ad?aƒÎñ–²?<T;µôåZ?aƒÎñ–¯?ï}ýZù?Ž<cÈ;h—?@]"¼€ð?Ž<cÈ;hŸ?ïùªÁ©*M?JQ–Õ­A€?ITù[VÈ?JQ–Õ­A}4FGL J0325.0-2416¿ï›ÓÅÛÀK³w ÈÍdÀ;[s¶±•À<µ\ÿµ@ßý®ÁôØ@]SG¥°ÿ?ÂÔé¦Í3пµ×"z,?òã<æ:\@hNAy¿Ìb{ 4hg¿è÷ÿ¶.$Ö¿á•+uϏö¿ïì;ýÝ?퓟ïôð?Ì7
Þ:ŽAGNfsrqPKS 0323-244?ïÿ†òŸr.?–£Tš,<?CX#ts•?–£Tš,"?ïþ‡i+¯?Adöž°,1?'‰mE™ˆ?Adöž°,/?ïË É J»?}6ý²å±?z/›/Ú¢"?}6ý²å¸?ïÿԏ{A‰>ù`â‹ÞÝY>õ¸B_:ÕÊ>ù`â‹ÞÜû4FGL J0325.3+3332?åkÝöçœÀ32|EÀ:ۘkœ0MÀ<(ŠÅÁ@@ÞÜØÞ}ú@Ñ1ìVu?ο'½†,?¾¡Åg}¾?ò¢}SõÌ@Êãés÷t¿ïð£5úÐ?ïýâƒî6ª¿ê¾ÝöÀ¼¿ÃË`æõ—ò¿æ£Ò½§•Ü¿ïÿ'ò¶kaAGNbll2MASX J03251760+3332435?ïñòãVøö?§C¢Èc?\9R°?§C¢Èa?ïÒ4yï5«?™-4
KHs?våÃe*f?™-4
KHq?ïT³öĪ`?×TŒUo?•i'j³å?×TŒUo?ïxSÆëå?ü՛Ë|?õ‡"Ÿ#d?ü՛Ë~4FGL J0325.5-5635?é†Ã÷ÓÀHé*0U2aÀ9ÞT8fxÛÀ<c!¸·l@¤&ó?þä¡Õ¨>?²@ÊžUì?£Sþk«?òTE·š5¡@´2vÐ?ïÿ˜ È¢q¿ß°Å/Iš¿ÜÚ\FQô¿á3ËÿY˜¿ÙÏ:û©"¿Ü£¸AGNbll3FGL J0325.2-56341RXS J032521.8-563543?ïÿ^Ö%vÛ?ˆ=S´t½?%;Q$•Ï?ˆ=S´tð?ïþÒ{`A?Hß&›‰.?/BØIü?Hß&›‰?ïòJíðs˜?jã³
g§ý?[j$Ï8?jã³
g§ø?ïý‡À›ì?('0ó‹Û8?7ãÁû Ÿ:?('0ó‹Û^4FGL J0325.6-1646¿èøá(õ
ÀJwÃ?…Q
À9'BG£-À;æ³ «Ü'@¡ØR¼æP?üÖ#l?¬bjBD¸?ª—ÁA;J@ìsƒ…[@
sd{ª›¿ç=†É2¿Ôëˆy¶¥C¿à-qÊÛ[¿ÔOóÞ3§w¿âEœÂC¿Ñ,`Eºõ4AGNbll3FGL J0325.6-1648RBS 0421?ïþnæu?#v6Ï^Í?)1˜¸•?#v6Ï^ÍK?ïüçE˜7?R)<ÿ¾	?8Å׃>JO?R)<ÿ½ù?ïîèáÅÝ?f1™7Óx?a:"í~?f1™7Óx?ïøýs	?@JUm™&_?LŸÂ3â•?@JUm™&t4FGL J0325.7+2225?îkÆ¢å`
À;ù@»±òVÀ8¢ÆÅKÏÀ;Ä"Ÿg8ô@G¶h‡Rð@K%}h
«?¨íöëÁÉ?ÅdI,@öøj	‰@²ÑÖKý¿Ø1—׿¿äª¿_»ý¿èwÓ«äù¿ë,L$Ì¿íîa«ì¿ïÿíöé	AGNfsrq3FGL J0325.5+2223TXS 0322+222?ïú3Ì8Q?E'X>ÝÞ:?G0Ï–»‡?E'X>ÝÞ0?ïìób¾Q?rÔ0¦n\?câA­8?rÔ0¦n\?ï
úsfì¤?•¾ÅQ¹?ž@±""k^?•¾ÅQ¹
?ï‹m¿,î?{+/ÜuT?$¸Ð4ÄS?{+/ÜuV4FGL J0325.9-1843?ê'ñ±ÈÐÀJ̹#¢œxÀ;³"â{À<‡¡†`@aA¹^@£BàO`?ʕΈ䕖?ü–"¨q?×jîöÃ@\@c±^²<ÿ¿å‰ÿ]BÑ6?ïÁÿáø¿é. À4
¿ÕHãß
>¿è^ëÈRj¿ÔX£š¤["AGNbcu3FGL J0326.0-1842PMN J0325-1843?ïԍ÷ÅÑ'?­Ò"hm ?u¹m$?­Ò"hm ?ïüŠü{KF?TÏfôèÉ?;¨%¥Äù?TÏfôèÇ?ï¼öieŠ?'¤—}`u?€Âe¿æ›?'¤—}`o?ïõ•H¥c1?G¼¤00'F?TÕnµ9œh?G¼¤00'=4FGL J0326.2+0225?½¢™ÖK"ÀE5¬îàóËÀ9RÁmóùÀ;ý'€ ¤P@ )j \×F?ý™SÃÌs?²ƒÆôp«?"¡q\í?îFTþ_@:;j?ù?êEXßÀ‹¿áp^¢LƂ¿âsEaÞí6¿Ô£,å¾`¿×²!vrM¿ãûbâMhAGNbll3FGL J0326.2+02251H 0323+022?ïýš'q?&Á~</å?3+ìw–D?&Á~</T?ïý¤Oðh?M'<u«s?2݀|¿5ø?M'<u«…?ïõõÉè="?]~8
E¸8?Tl/"Ú?]~8
E¸?ïðã28X?IBïÏ-A?^8ߛPÁ?IBïÏ-V4FGL J0326.7-3404¿×0òÑIòÀL	U`"¥À:ÖõtŒÀ<Æ$)ªô5@^ê˜Õ?þb,•Š@`?Æ(¿ý0—Í?É(Äûb7@C]œ"I@éj£·Õš?àMÍþ¦
Æ?â$EÅ.…±‡!¿ÞÉÖço¿ìÏ‹¿¼¿­"ŸÚsAGNbcuNVSS J032644-340330?ïÅ?–ˆ¾?vb§®¼®4?}}à4» ¾?vb§®¼®5?ïûƒ"W}6?XCœ€Íç>?Aóv¢&d?XCœ€ÍçG?î8,('?¾–F¡÷?¬}=}Žn¨?¾–F¡ô?ï¹¥6yUò?pJª¾T?–²aªƒ=?pJª¾T4FGL J0327.5-1805?òÈÛþÀJrGE8ïÀ9þ\XÆj³À<3ë‹Ô´ù@ñÓ"§IÛ@‹ÞZ"ÊM?·Ý­DÇ/T?¹@1¸#?õõƃÝp@Ä E°8m?§9ÓtÝ¿è	N}'{=¿ìòwéF¿ãˆ$&Oõâ¿ëñ–¼ˆÝ¿ïþùÀJÞKAGNbcuCRATES J032743.34-180342.0?ïþ/[AÂn?8Ã0CJvá?-
KãÙI?8Ã0CJvÏ?ïþ¬&ˆ$?CÞ²:¸HÞ?%?½—}Ñá?CÞ²:¸Hý?ïѓ ?{Xú¤€®¾?w6?qu0a?{Xú¤€®¼?ïýZý¶?&v³EÃS?5+2^Ò?&v³Eô4FGL J0328.8-5715?ØÝ[ñDDÀH‹¼¾aÐÀ;žJœ	¶À<ì^ª°BS@"t˃÷q?ñ×ôH;Ù?äoñ•1ä?á—Ïà'~@˜"?úJVËhɘ¿ïå¿Â£(9?ï–Á¥)ñ¿äÀ€æDm¿Å3ÃçJýT?¦à±[,K¿é}"€U$öAGNbllWISEA J032852.69-571605.5?ïâO%\:í?ngmᓟ:?m°Ú£Å?ngmᓟ4?ïìˆý»?‰B)è‹Ø?cwèïE`?‰B)è‹Ø?ïfõ¡?‰"‡óš?¦B»—¹Û?‰"‡ó•?ï°S`:ò?{™Ë¤±t?ƒý+'ñC»?{™Ë¤±r4FGL J0330.6+4659¿Ã¹TºôÀ™tNƒÀ9•¶åû7À;ÀcK(ó>@<8?Œˆ@oÐ!ëã?¾ÿ·ZʦØ?Ä/â›Á-@Ɣ‰`[@g+Þ*B¿Í—£ö¿åz¡–'õ¿éÎÚÄT®¿éêÿR[§¿ïóȟ@¢‡¿å¶]õ~AGNbcuB3 0327+467A?ï³?@æY$?‹8?¾–[?ƒ0/Æi¶è?‹8?¾–\?î\ÇÃÿ¿?¹t᭏ˆ?ª3ƒÀ?¹t᭏ˆ?í滊ð˜'?¦|›¸ï?°Ê#¨{;w?¦|›¸ð?폛ø‰@?šá9Ô:÷?³‡K ;µþ?šá9Ô:÷4FGL J0330.6+0438¿ìÙGÿÁiÀDã>ÿPÀ9Ï"M1âÀ<%E«Hï@»ƒú @DÀßXÀ‹?º½<áÝ«?¿C¥`$Õ@»­À˜$@十×?ì۝_¡Ñ!¿´&,9™Ô¨¿æŸ³%]¿Úþ$þ½	á¿êý՞,¦Q¿ðAGNbcu3FGL J0330.6+0437GB6 J0330+0439?ïôy¼¢M?UÑ &¦?WÃ†»d'?UÑ &¦?ïý Òπ•?I2´Þ,¢ ?2ùiƒûP?I2´Þ,¢'?ï?ÁÖÃË ?"­"ß%î?˜Å'†‹ß?"­"ß%ì?ïô'1¢??I3F7Ó$?W±œz»•?I3F7Ó4FGL J0330.7-2408¿ë½š£Oó­ÀK82vtÑÀ;b«ð´2¢À<Ù£€£(@ *Ï·bØ?úM "Ú?Ôä< DXŸ?Ïpk"ð(?ûãèrDÁ@ƒ¼|±¿ïʒ€Ê÷?îrE ¿×¡P&kú¿ÒtZÅÉM¿æzÐKŽ¿Õ>ê šªAGNbcuNVSS J033050-240612?ïôƒtùü8?Rñëx¼lª?Vù"D?Rñëx¼l¥?ïôºªÓD…?tO–X…Ð<?VŠªYv÷V?tO–X…Ð=?ïº"O!?|d[Š}®è?wl7Ÿ½5?|d[Š}®ô?ï¹$dŒß?qҁ™˜†?¶üæÜÈM?qҁ™˜ƒ4FGL J0331.1-5243?áµ·ÁcÀIsüC²Ý7À;&ê«Úä¾À<ÃNÂò®@H‡r¦@yýåsŒÀ?÷øX$Ú¿š÷•ì¼?Ô©S æêÛ@É(Åñç9¿ß˙‹í¿âþP",O¿¿é'A¦"} ¿àXÍ¡ˆü=¿ïÿý±q&´?äQªí~ôAGNbcuPGC 013066?ïý¢ZØÓS?4·| àÉ?2í)9eo?4·| à¬?ïú7'/þ?]-£yE—¸?G!»Aøš?]-£yE—·?ïàO«¢èô?oÉÄ¡b$?o°T]ƒ?oÉÄ¡b?ïü•¹†ù?2-ñR{WA?;R3È7"H?2-ñR{W14FGL J0331.3-6156?ëÛÀ8!GŽÀG(µÃ›Ë£À9Yėt%À<Jè:@X+ü2@?ÿbBw†?®™½
ù#?°êÀŸÃ@¥:œ´M@¨]e‹Êú¿×û_1hÙ¿~‡€££¿ÞÖtD¿áÀmä	)t¿áæ!‡+¿ã˜r‡ÜØ´AGNbll3FGL J0331.3-6155PMN J0331-6155?ïý²ÑLå–?)¼ulD1?2iu˜ÓS¿?)¼ulCí?ïü¬M¨Æ?[Õ+"m}?:'¹Ðæ?[Õ+"mu?ïæÉúlí?o)2f´È•?i6"<S:?o)2f´È¤?ïí˜X6å?R"ÿÙwW?bg§Éï‹?R"ÿÙwW4FGL J0331.8-7040¿éâ큙=ÀD{tÝÛÀ;ç&ďçiÀ=©'^aµ@"ÙJb¤ºà?Î*ÚI7+?ì?»×²?éóœDnÄÚ?ýâ©Ô#Ù@í§d2"¿ï÷[0H¿ïOµIùHV?ïé !óð¨¿èÝV‡Ì¼?Ó¢=ëó¿ÊAÜCbUAGNbcuSUMSS J033202-703952?ïçTŒlEÕ?là4,§?h«s"º*ö?là4,©?ïþ8e|Z¿?EÑè="?,y¨:TÔ?EÑè=Œ?î†þr¢Nm?œ{ÂÞ®g?§ÕÛ*?œ{ÂÞ®h?ïÿ²¨Ò~?%óÜÈÙ"?	ªå°H{?%óÜÈÙX4FGL J0331.9+6307¿Ã•žð`y@Ç€¾À9*æ?d™ÞÀ;ÎÔ°ÆÜÉ@×ÍKͳÒ@4dÁJ¸‹?²vNÜ±œ?¶Mp÷ê@WZYèª@	¸¡"Ä"¿Éëð¾ïi…¿âLð=ë¿Þ[^Ëgqÿ¿â‰Úßµ¿âú1T5â:¿ÔHþ¡†"AGNbll3FGL J0332.0+6308GB6 J0331+6307?ïõùðŒ?O]àÕ?T
âØë?O]àÔö?ïäSñ‡Óm?ƒÄãBMqX?k¬x,'÷?ƒÄãBMqX?ïÓOÁ<"2?yŽåÜڇ?vXaµæŒ?yŽåÜڇ?ïj`Rô£?}˜7h9œ?'³õ¡mëo?}˜7h94FGL J0332.1-1123¿îJ¨hãì¯ÀH–s-õÑÀ:Õѧ' ÖÀ<lšu%F@¢Ä—ôþÅ@´L{՝?Õ%
¦w?؆B#æäü?þÚ®½M$@Ž¬7+¿î9_^4i?à°ïÁÄ[¿á¾Jô°¿è¸uAË|¿ïþ0Q×c)?ïÎ0Ö¯ÐAGNfsrq2FGL J0332.5-11181RXS J033223.2-111938?ïø
¡È'd?XLºáÙ|?OÕxÝön?XLºáو?ïü'-Ú×D?W/œêÌY¯?;v')E؊?W/œêÌY²?î-¹;çƒ?šYQⰒý?­$lAˆÕ?šYQⰒü?ïòÜYÀР?R€ÍE"€Ï?ZGL~^º?R€ÍE"€Ø4FGL J0332.8+1557?íËu¥çlAÀ?È)ˆ;£À;H™Ì¢ÛÀ<ŒÎóº1@ fWÎ.å?úàSý®(?ØÞG ÏÄ?âc¶ˆ½©C@ úÄV܆@ü0à¿íèÐ~]($?ïÙQu=™¿?…Ñe¹¿Ö—¼Ô¬j¿è¦¸f
{¿ïü¬ÄÉ%AGNbcuGB6 J0332+1556?ï°9É-T?‡*;§«h¡?ƒñ´ªý?‡*;§«hŸ?ïß\9õß?‹þM¥W›?pQãwÏ?‹þM¥Wœ?îŒf¸—Ÿ?®b_áÆ?§9"v†¯?®b_áÅ?íê*Z"(÷?¢V:l˜?°®­+Þ¸D?¢V:l™4FGL J0333.1+8227¿éðX(š@5IPüqÖÀ:ÀAFmDÀ<¬Š‰[]õ@™Têèí?þC:sÆ?Æï¡
+b?Ëyˆ'!@®ŸÀ@.وœò¿îºadw?ïù·a*½C¿ä<Í`pƒ ¿×H¢L@¿â¦wÎm·¿ïㄟ6'AGNbcu1RXS J033208.6+822654?ïßèöó'?nÞ7ƒÕ¥¥?p~"†>C?nÞ7ƒÕ¥£?ïÞ2žp ?Œb$¹y?pæ°¹Gï)?Œb$¹u?ïFlÂW?'<'Å(ý?—2~'µL?'<'Å(ý?ïž+¯®à?Š¶Û½¢¾?ž:Š
$:?Š¶Û½¢½ÿ4FGL J0333.3+0233?ïóà¯Ý¹ÀD~~¡ÆÀ;a .QÀ<‰<
ÍH@ GRBBÖ?ú{R¡ƒâ?ÒÁÐÅTÞT?Ôø'Äj'¼@Œðs›O@¨¾vÁ¿ïþÃÎ!a?ïò¦Ey†Õ¿áËZ§ƒ¿¾p¢ÕWŠÖ¿ëÁšÀ«¿ÕÝC<•²"AGNbcu3FGL J0333.6+0233NVSS J033321+023110?ïüv<Qï?B°·ô,Ë?<N%pe?B°·ô,°?ïú‡¹áÙ?ad"°$>²?Gõáx¡í?ad"°$>¯?îÕ³#þ¾†?–×·¤
ïÑ?¢¤ÍÀŸ?–×·¤
ïÏ?ïÆýz•³<?sçö;[i?|Bµ&`É?sçö;[g4FGL J0333.7+7851?Ɲˆ
Á2Ø@2vF¿2/À9ƙWTz¬À<f£ÝÀ:@Ôµ'"™€@ÐÞªDã?³PSÕj*@?¯Cûq??øùìU(P@æ ‡4U¿àQž®+w¿Û˜0bôA¿â Ð$p!Ñ¿ÜOþ$ކ´¿á‡_<ü`¿è´À}‰AGNbll3FGL J0333.4+7853WN B0326.7+7840?ïî‰;®7A?aVƒ@±»|?avÄQȾ»?aVƒ@±»~?ïöÝ®2ƒ»?j2\KsŠw?RD£šøŒ_?j2\KsŠv?ïÜ£%Ã_Ó?{:Xµº!¿?q®mP¿?{:Xµº!¾?ï"!Ÿ8NV?t3Œ?¶‰Ü?‹7˜1ìj?t3Œ?¶‰Û4FGL J0333.7+2916¿îþü­I£À5êÝYÀ9óæí	ƒÀ;­	¾º@U‹DÂ&×?ýV‹@š?­[åÂâØ?¸Ñ|ŸbÜC@‰Oâ–b­@—Ñ)(¿Æ­þÖ_G¹?àµbîᶿޛ¤¡4˜Ž¿Ø?"Š¾µ¿äg8ô=T¿â;ÊYêWAGNbll3FGL J0333.6+2916TXS 0330+291?ïõÙ1¿Ìý?S)Z!h?TMœ€f?S)Z!_?ïµMˆÎ5x?šùV;A
?'¬Ìr¢?šùV;A?ï|Ê1oÉ?Žßi݌&?f¹ÒÞm?Žßi݌"?îREf½{;?'ÆYÐG1?ªÛ©"(LQ?'ÆYÐG04FGL J0333.8+4007¿î"®åÎÁRÀ)Á%µ¿jÀ:žjÇ7#À<^/",z²@ÅûÍ@@yƒœS?ƃuÀÌcp?ÂK´^kñ?úOfÛl7@…íë*†¿ïôäxºüÁ?ïû+‰>¿â: D®…º¿à¸‰9˜¨¿æX'r0t¿åPJ9ßöAGNbcu3FGL J0333.4+4003B3 0330+399?ïóì÷²ó?Zœ÷,8‡T?X'К?Zœ÷,8‡^?ïù­®ÆvQ?dlÁŠx?IIDæ&À?dlÁŠv?ïÍ$Vöo§?yx.¶Û?ymԄÈ+ê?yx.¶Ó?ïª]õ/]?t40~'?…h'»4)?t40~"4FGL J0333.9+6537?ììåc›x]@^ ƒxÆÀ8üƒýP"WÀ;×ÛIgR@ \@LÌ6z?þ°®‰ç?­9Cm"x?¯j*$@Á@y¸_~@°E
%W}?ìêKBž‹¿Ç
A\Õ¿Ü*¸$õõ¿áÝÖ´¿Úr
žêff¿á!ðÐrAGNbll3FGL J0333.9+6538TXS 0329+654?ïü,PÃ?<ú]í??¡ç•?<ú]í?ïôºQ¬?pÙþ!`Ù?Vދ\Þ©•?pÙþ!`Ü?ïÖlo/°Ð?xªéÆ*ÌO?tÉÈh'˜?xªéÆ*ÌO?ïçՙ;æq?Vf•Äߎ›?h*fďZ?Vf•Äߎœ4FGL J0334.2-3725?Å©öšZf¨ÀK1–¦ ZÀ8V(LýàÀ;ŠÓ8÷˜R@vz†.?þ§]§{¬?¡$Xyé¥ö?±gýí<j@«BE@i¶ÉŒ&¿Ül—B|Q_¿Ù}Ã@1¿à_ÿ¯x(0¿àªjl…dX¿ãÑ}ÁKå1¿àŸì.'ãÃAGNbll3FGL J0334.3-3726PMN J0334-3725?ïÿÕN:?Wã
à¢?eV<¹ü?Wã
àó?ïøde&ÂÃ?d|ŒÛ^³Ä?Nnkdôö~?d|ŒÛ^³Ë?ïÆÛF© ?ƒ*—K€5?|'}Ü«/½?ƒ*—K€2?ïöÂî¼¢Z?Ac ñž5º?Rz"†»M?Ac ñž5®4FGL J0334.2-4008?îÑÜߙó˜ÀK	ˆ MÀ81"+sKQÀ;¶½-˜½@'Y‹b@žý¼XáC?—‡>¸…:?²'T>×½R@œ
²p*5@µ‰ÐMà´¿È÷Œ¾ê¶î¿ÜãÝ Á¿ã"õ¦n"¿âáÑa*<¿æà¹(«¿è à¨-±AGNbll3FGL J0334.3-4008PKS 0332-403?ïþè$Jtm?G—RÚ¼?!}»X¹#á?G—Rۇ?ïõG?ÛýÜ?lÍ0éï-?Uq€HE†?lÍ0éï)?ïãÑß
ý%?s¥Ï7hç?l. õڃ?s¥Ï7hç?ïþî0Ø8?L!à]à?!,ò|€q?L!à]à4FGL J0334.3+3920¿ï	yHoÌÀ*æèÑQ­À:½lŸe‹uÀ<rüp(‡@!"nPj¦'?ý1?Þ<`Ù?¾%vkí¿"7"îfÐ?Ö¨"s¿ë=@3ÈÂüê¿ï¹¾GMò?î÷L!ìŽß¿âZr¦æ‰¿ÑuºÆ"$¿å˜<8d?¥y@ޗz†AGNrdg3FGL J0334.2+39154C +39.12?ïþ_Hp?!…2}5<Ÿ?&*‹yÛ?!…2}5<=?ïý"Üäýr?R˜Bmw•?3YØs'?R˜Bmw•?ïóGeË?`üíaëû?YÍq4ió-?`üíaëé?ïéïƒJJ¿?^Ž
–r ä?f|µµA?^Ž
–r Û4FGL J0335.1-4459?Èü‹ã°îÀJwŽ}ܤ±À:¹é›9­À<z	d,ÐC@¼ ý¦‰l?ÿ¸ŸõÔ-?±êUéŸì¿R 	äôû"?œ,=mO@û5ëÊ?ïë}[‹¿Ìi"ïî¿âç&J¤‡¿à`ÃY†"¿Õ:5ÛÚð¿Þ`¸vÔsAGNbll3FGL J0335.3-4459SUMSS J033513-445939?ïý|å1Rý?0Ð;‡³?4ÖuhP?0Ð;‡²¾?ïþë ¨"?9Ê-)u•~?!MõvÆÿ¢?9Ê-)u•Ž?ïò[ l
ô?f›ê—UOÂ?[H¿'ä?f›ê—UO¶?ïÿ#|'œ?p³Õ?|¬'Ì?p³'Ï4FGL J0336.4+3224¿ÐÄfðñùCÀ2²býüÁÀ9èT菡À;ƒT¦Ë±@ÓÝ@ß'T·?¼éÝú'Ï?ÞV›Ã'@Õ¸ÜU
@¥Í¸Úýg¿¸ó3hãi¿â1®~-,‰¿ë²¶°*Ö¿ïîªm&t?ꋪ=UËä¿ïïë L'(AGNfsrq3FGL J0336.5+3210NRAO 140?îf^ƒ`ºh?Ál&nšy?©šÉôY'?Ál&nšy?ì϶Âńõ?Ìĵ)óG#?¹'IéÓØY?Ìĵ)óG#?ç<K0M¥?µ<€
uW?чiߟdµ?µ<€
uW?í†r›ñ°É?³'ýãjž?³Ìk ryº?³'ýãjž4FGL J0336.5-0348?ØñœÖ9ÀF—ædNÀ;Eag°À<JFu/W@"pø¶4¯à?ùìl5ç?ÉmŒàΌk?ˆÊ‰¦‡hÀ?ÁE‡ô€›?ÿ¥,ŒûÑr?ïþ¹^Zÿ*¿î' ×?ªqDC"l¿¿ÛfwBוÿ¿ÜTÙv({?»±Æ¡‡GAGNbll1RXS J033623.3-034727?ïÿ~x%ü?yÅ»Ÿ?0û@nkÀ?yźÁ?ïý
BÒb?Q={Á!"?7•éoüâv?Q={Á!—?ïóxwÈö?`#<oˆ˜|?Yûn
?`#<oˆ˜"?ïðyu"?QjïË©"?_
Á×ÿê?QjïË©ƒ4FGL J0336.8-3612?粬ÃI"©ÀJ÷¦a(9À:DՑ—l™À<m?æŸÜª@ȋä¥0§@[Ò#Mââ?½":'x5?—³HG8ñ?Õ螄ºåD@<¶a{p?1‹"G¿æèG]ÿ¿æ¨Š'¾Ú¿ëpê7.j¿ïøp¿…¼m¿ï÷¹_‡¤úAGNfsrq3FGL J0336.9-3622PKS 0335-364?ïüb"²Hd?@öO&¦}?<ëbm¼äp?@öO&¦y?ïÆ~™•?ÚðñfÆ?|À³5@€
?ÚðñfÈ?ï§ÞØ1&µ?†Å<5Qá?†Ió¶R±?†Å<5QÞ?ï›{J`?yùdƒð`y?‰!-zgú
?yùdƒð`~4FGL J0337.8-1157?ߪfï"mLÀH
A1"¸À:ž¼Õ,À<_‡ÚTtÌ@,³‹™Q@ž/Egé?ÄaJȦ?§ß"\BÃk?á"Ì`it@Ðú'­Â?î@aNÏpì¿êÈ@Á;I,¿äD³zì¿é¨aé)#æ¿â¨:{üС¿ïø¡œZAGNfsrqPKS 0335-122?ïúŽœ[UI?D˹Ôj½?EŎ'ª×ü?D˹Ôj½?ïîÕ6½ƒ&?xUä°ƒ×?a*ÉB|Û?xUä°ƒÕ?ï—ôæxoÉ?ƒÕ/?ŠÆaä
š?ƒÕ/?ïÝÔ	"`µ?`\Q†q³?qû5Ï¥I?`\Q†qµ4FGL J0338.1-2443?àñ/HûÀJNœË}AtÀ;r–ÇWBÀ<¼œe%ô†@!óx"9®"?ûp)þ×?ÉÁ`ÝæO«?©Ü½ýôY{?äáý€É¾û@w{	
À£¿ïÜT\È?ïŒD±à¸<¿ÞaÁæê°¿ãáÍzq¶&¿æð莐§?ã笁Ӫ7AGNbll3FGL J0338.1-24432E 0336.0-2453?ïýÒ|Cќ?/îd¼=I#?1lásk?/îd¼=I]?ïø¾'¹Æî?j$Ðgƒ]G?MaäJ?j$Ðgƒ]P?ï´7#º7?"&OITë?'ò7r:u?"&OITí?ïæP:…Y?e¨f'Óß?i¯ïÅz§y?e¨f'Óà4FGL J0338.5+1302¿æZóSZ-2À@w¼Â"çÀ8ÖÛjËÀ;~$–¸=Ê@ K	óô®é?ø"ËßgD?±2jáJ]?Å,Àþ7~@ßZ',•Š@=ZÿU
¿ïÿæj,Ą?ïÿô¬å¦¸¿Ô5Wû"‹h¿ÆÍ7€ÊÀ®¿ßaŽû°åæ¿ÜB"dXðAGNbll3FGL J0338.5+1303RX J0338.4+1302?ïåTx´K?oóÁ¢åØ>?j«‡ùK´–?oóÁ¢åØ:?ïäWäç?Ïm—ä‡?k¨ðý?Ïm—äŠ?íü{–‹ðæ?¤½Ç½í6 ?°#K xÍ?¤½Ç½í6 ?ï"z f…?‹£™ãRù?›°«ó<?‹£™ãRû4FGL J0338.7-5706?ïÿNöÁÀGþ+@öjUÀ;ø|·
èÀ=,:ñn@"ANoÑI?úç5ï¦?ËîÂÖSß%?–ï(lZÇ!?Í ÓŠ+<š@.Õ>5p¿ïî4[Q_n¿äùp~î©?ïþ$'ýu¿ÓÄ­ÄsâÑ¿êýOa<é?à@¿ºAGNbcu1RXS J033832.0-570449?ïÿI¶r¬? :æÀ'¢?É1¼j€ë? :æÀ'Í?ïýéÝßüû?FëV.
Ä?0±-Í?FëV.
Ø?﬇eÄ ?†W€[çÚ?"ø^&ŽØ??†W€[çÜ?ïúñá$^š?DKö|cl?D8{n…˜ö?DKö|ckî4FGL J0338.9-2848?ê#m­pâ¿ÀJ"K±¯:À:ŒAœƒÀ<^.bT@&n¿%oP?ÿ…1˜(€R?²#M"M2¿—Ÿ'ya7J?èrŸæ¿@àP64?ÁH½Þó@¿âXœ‰8#¿â@^"àÍ5¿ß	Ñeõ¿Ü&D!íæx¿ÆD
›åNNAGNbcuNVSS J033859-284619?ïþ°B¿=?âÿ·üÿ#?$ûÔü/?âÿ·üÿö?ïþT¯Ä)?E" 7¿J6?'
µ½u£?E" 7¿J9?ïû/Å
Z?CïS§$•U?C@ë֗þd?CïS§$"ì?ïþêǬÅ5?
ÅÙT"Á?!S…3¬¯^?
ÅÙT!·4FGL J0339.2-1736?çћÌcè€ÀIG"#ÐÀ9•²F8ÉuÀ<\ªûÁ­@†rK!œ?þd¨Uôÿ?°ÍÂkØ?¡ØÎbÏ1?ó'
8ͦç@w|üTú®?ëpø@¿Ð‰§»§¶¿áC™b<5:¿Ø´Ó[Ý '¿àÇ7—FC¿Ý6¤!1þÖAGNbll3FGL J0339.2-1738PKS 0336-177?ïý9WøMÑ?+œÃœ×ˆ?65@='| ?+œÃœ×ˆž?ïý>ÇqrÁ?OŃÎlu?6	ÄtiûH?OŃÎli?ïõ3·÷7?`Zø@Ü¢ç?U™È'¨?`Zø@Ü¢ß?ïíÆ¥œU?P@8Û?b9Zâcª?P@8ê4FGL J0339.5-0146?ì&ֆêeîÀE:h±šA_À7qëýê|
À;gKoj'@
Qg¦­S@ðÜá?'Ö•<VŒC?´Ý)¼<ë@kMHˆ/@EµªœK¿ËûŸú[Ñ¿àÍìlø¿å€…áÖÊ'¿åÒBW"¿èæWbg~>¿ç]™£ª""AGNfsrq3FGL J0339.5-0146PKS 0336-01?ïñHm»~y?YmÁddÀ?]o$‰?YmÁdd·?ïè¡ÌN¢?J§Øõ
?g^3±]ïÊ?J§Øõ	?ïǤr¤"?|1ÒÝü¦?|-ÀF­îž?|1ÒÝü¦	?ïülX:ãØ?3qäʖ¥?<>(á;–?3qäʖ¥4FGL J0340.4-2422?Æ_Ǧ'1ÀJ ÝDÀ;ö,A§jÀ<»UãTÏ@ Oa<0?üz0bžZÉ?Ñú¦]Í;?Ù9Ã¬è@$ž¶,?ú©W³è¿ï×+Ë_åC?D8>5?łZ7Ùá¿Ö~œÚñÔ¿é5­@ÀdŠ¿ïúö`™ó²AGNfsrq3FGL J0340.4-2423NVSS J034022-242411?ï'3YÐYR?løìÎ;k?‹s)‹é«š?løìÎ;j?íôª‰dW+?¼´;μ¢?°Z«´ÝF§?¼´;μ¢?ìé'ðØÑ
?¥à£÷ç΄?¸³hy9w¦?¥à£÷ç΃?èN'[ܧ?³öö&¼Ã?ÎÅö…f?³öö&¼Ã4FGL J0340.5-2118?ï¢ÒjcÚpÀI–Ñ¿zÔ²À9E?']<À<Ciô`@©÷è‰ø@Á°9ï?ªî^å5?°0Y9(Á@'ÿœ,ñÑ@
Ê*uõO£¿¤øÜc˜¬¿à@úœðž¿äÿT¿:¿åqøÀƄ3¿à]s]Å­õ¿è ;tJT¸AGNbll3FGL J0340.5-2119PKS 0338-214?ïýÏEóg³?+˜¡˜4f?1…ÐdÂbw?+˜¡˜4j?ïý‹	øã ?Qt¸6§#{?3§°8ãl?Qt¸6§#}?ïä¼y3ðk?n'Ñ—K\û?kC†Ì•<?n'Ñ—K\þ?ïô•Ÿ È?H'qJsã?VÔÁ¿ômð?H'qJsÌ4FGL J0340.5-0256?áLèv¥âÀEtžý†¨üÀ:ªÏmýÀ<Ybцoñ@'{^p"Ó?ÿøŽ‡à?ˏhc?Ñã<$ôV)?ý
O#SÂ?ÿ‹çýÈ?ïõøÀ·¼¿ãí¥Ùÿ¸…äÛâ>y¿çƒ¿ÝÑ¿å(R. ý¿ïÿA^o! AGNbcuTXS 0338-030?ïÜs.žîB?qÛF†§Š=?qÆh°ˆß?qÛF†§ŠA?ï°Jëvþã?'Œ¯:d?ƒíE"@Gb?'Œ¯:d?í¾s€šY©?¡ôš"Óy?²cû-2Â?¡ôš"Óy?팗)€%'?œª'Ú–æ?³›F³þÓq?œª'Ú–æ4FGL J0342.2+3858?Ä:™*…û%À)˜øçÝÊKÀ:QÝIÒÄÀ<9à+Nbd@9ºZ.t³@üº€™îS?¾–y(µÖ¼?–Úâ}ýˌ?Õý†þâHµ@NžT¿J?íó
¾¯}²¿æ4M¯¶;'¿å¼ùðòF¿âˆ^Þ²¨¿âÞsV–¿ëšŽ ¿"(AGNfsrq3FGL J0342.2+3857GB6 J0342+3858?ïþ±¬8f¨? ñ!òhì?$å<y•~ì? ñ!òhà?ïþ¢¢Ù¿?BÙÄô¯˜ó?%ÕÒd?BÙÄô¯˜ý?ïõ–¼0|?_ßGI(X?T҇ϟ¡?_ßGI('?ïÿ°š™Úx>õfBÀf°Ñ?ÙY‰aì)>õfBÀf±4FGL J0342.8-3007¿ÄõÑʟjøÀJ>U⊤3À;\ù1¯¥uÀ<è~ ïÏ0@|ØãÀ¯?øï»åüj?Ý儠¹?ãJB¾ìdm@ l‡י@Úën"d¿á²ý¸ýâï?ïÜ¢ÍõÁ¹¿Ô—€DY¿×Aß3ÞL¿ìŸ_¬8¿ïòÛßå-lAGNbcu3FGL J0342.6-3006PKS 0340-302?îÖ¶"ξ?¡<9‹Tö?¢"–Ã$2?¡<9‹Tö?ïÄ+{­•À?˜ý,A~?}êB)5€?˜ý,A~?íWÕÑO? ëþ‡ÛÔ?µGyW)u? ëþ‡ÛÔ?îl0÷ý?˜V±"¾˜O?©>ÌðŽ2?˜V±"¾˜O4FGL J0343.2-2529?ên*åÑ_%ÀIÓ|ÌyÀ9ÊdpÂà»À<d‰éù-~@Pm"½¿i@±oɼw?·*Aë1è?Âo'Ÿaµ@¡âއ	t@ҏe?Ô‰[l¿ä\¦(ô¿æ߆ôÛ	¿èq¼Û¾¿í2ê£whí¿ïüwIãxáAGNfsrq3FGL J0343.2-2534PKS 0341-256?ïùôgVg?Cª`Þªü?H.b¦cŸ_?Cª`Þªü?ïýIœð@Ü?P…5<Oò?5³}ùŸ?P…5<Oé?ï³ ˆÛå?€œMЇ–`?ƒÝÉ8F¦?€œMЇ–a?ïþ~'º¿F?êKu\?("T®i?êKu\}4FGL J0343.2-6444¿íÈBYӀÀEÔa¿7¸ÔÀ9y'S+ ?À<Sá,Ö"@ýt»¾³@	…º¿"?¬IƝˆ¼}?§áUšç!?û'YY7©º@Çl½Ãp?ï ±ád"¿È™òD€"¿äCN¾ÿږ¿à`)k3TÁ¿çí¸4Sſײßð–AGNbll3FGL J0343.3-6443PMN J0343-6442?ïýåZBaž?-—ØÜÒÜ?0Õ-ìó
_?-—ØÜҏ?ïý¼=ŽëÁ?Kl£1Ì>?2ˆ¡û3?Kl£1Ìi?ïÕ{¼Êâ?w/èþi¼?uB~¡šB?w/èþiÎ?ïý0á±à?)šU"¬=—?6x÷ºpöþ?)šU"¬=j4FGL J0343.4+3621?ì§þ4CÂ|À-fãOÆñÀ9ð¿§J\EÀ<jÃQ#@®Uÿfþ@€W$'°?ĘvßE?ÃÕYä!þ?ý&¾æZ<Œ?ÿe*ß|¨¿Ð"á+~‰¿é¹vCS;ç¿ÖÄO»)6Z¿çqÿ Üï¿ç
J5®7¶¿ïëa½µ,ÈAGNfsrq3FGL J0343.3+3622OE 367?î;Ü%MÑ]?©‰ÚtŠ¾?¬B=«"ê;?©‰ÚtŠ¾?ïeì£g­v?¢È°Jœ?"Bk"
Q<?¢È°Jœ?íEqØg?¦™}Ë?µÔq<Ã*?¦™}Ë?íVÚáf~Ö?œ˜z²Ñ?µI(ôÌ	P?œ˜z²Ñ4FGL J0344.2+3203c¿î¢jÛ¼À1ìP½‡µlÀ9q±6nQÀ;5º‹¨â@ÿúPh£-@qÅìÞ»?בÁŠúD?Ý×°UÁG@"˜Ã°ÄY?þÎõü›ò?陊€!"¿¿T³.@/¿è«ÆÑá	¿ë!jÃQ#¿á0–5a
Ý¿ïí%g˜•ŽAGNbcu1RXS J034418.2+3209030?ÒoÚëíA-?Ðè^?à)?æÈŠ	_i?Ðè^?à)?»uǦt?ÅùÇ÷q?ìžÿÑG3?ÅùÇ÷q?Ö8åIq*}?»¹¼ÖV?äã[GjÁ?»¹¼ÖV?Œf1Ï^ÚÝ?"ÍòŠ7l?ïŽg8"•?"ÍòŠ7l4FGL J0344.4+3432¿Î&Væ"ôÀ/ô‡B_À:ÿ@ÿ¤À<ï< @!v_[…6á?üÊÙþ
·y?ƎDÑÁ(T?ª‡1j…@?å‡q^-O@WDŽ¥J¿ïö«!ÃI?ì{Ϲçû?È6â?OÌ¿ÐÑLŽNý¿æ¼Áò~7>¿²PÂæ$AGNbcu1RXS J034424.5+343016?ïþ]>4Ë?'åˆQ|?*,¾SX?'åˆQ|?ïý'T¦
¨?Vbì‰Ó[?6ÅZϒ¾y?Vbì‰ÓP?ïé/zÜgm?qd"õ­‹R?fЅ#˜"V?qd"õ­‹Q?ïâ…ñÙ.£?`úÍ\?mz&Ñ\û?`úÍ\‹4FGL J0345.2-2353¿ÅÑcE#-ÀIj³=¯øÀ9@ßìdAÉÀ<Dªùš‹@ƒ°f·š@G÷`MÉ?ªÐÌ`Á5ë?²¿ïn¸D€@P<Íæ¨@	n£Rÿ•¿×˜ÑÞ«Ü¿â™ð‡Ôö¿ç¦]¨R¿åˆGä¿äÑTá®±.¿ïÿù_|è3AGNbll3FGL J0345.1-2353NVSS J034518-235218?ïýÍ»Û?0D¡Vã"?1—×"!$©?0D¡Vã ?ïö"<Á?l¶áîî?R÷‡þ}Ïp?l¶áîï?ïÚ¤Ù[?t'é'}Š'?r­"Rst·?t'é'}Š%?ï¿ï©PŠ?o7âÿP?€«Ý|??o7âÿX4FGL J0345.5-3301?ïD­j'ÀJeè'%À;(*FûgÀ<ÇMé—Þ®@åכ‡Û@lCõù?ÆÐ=…³:¿'ÈZ]É?Êá|œ³ªg?þ|jvìEŽ?ïÇ@f!¿è¢®Á¿ãq•+uпæ£Þ+™á¾¿ÙòÑäcÂG¿ïó²I"ÇÉAGNbcuPKS 0343-330?ïùSص?D|™ò/Û?J³¸+žÎ?D|™ò/Ì?ïñ}AM%7?uè¸:<yX?]}eµé?uè¸:<yX?ﻧÔ?z÷'@?<
ø:…?z÷'@?ïè4Z¶Ûå?X| x'é?gË¥I$£?X| x'é4FGL J0347.0+4844?똅§²AÀg|¯Ý©À:tü+_)À;¥ðFN™@²Æo­G@©âå=?É?:èß'?Åu°†E)?ù´…xze!@Í~¦#?Ë?æm®YD>ô¿çnµŠè¿åK—"pî*¿ç—IBi1¿éöÒÅ4R¿ïþ YQUAGNfsrqIVS B0343+485?ïÍ	§Lb?x¡«éáQ0?y{,YüÏq?x¡«éáQ0?ï÷¨L
c?r"Éó'˜z?P¯gë9úÛ?r"Éó'˜t?î¡ëhÎOÚ?˜Y|»Î9?¥áIs\?˜Y|»Î7?ïžÖü¤µB?p_²ñ?ˆJ@ÖÒ¯W?p_²ñ4FGL J0347.7-3616?窅Z?άÀIÞÿ´€¦À:Жï›-îÀ<¶¤À>I@ý"õ•Ä@"÷H¡Y?ÇàV
??¯¬3á?0Ô?á|tŤº@¼dkd}¿åÎÃ|Áò~¿áŽ®žä\6¿â÷®aÐ*¿å°B½ê±º¿ä•^Pp¿ïÿð ¼x—AGNbcuPKS 0346-364?ïÿ¯;ÇXŽ?¶­µÔMm?1)ÜûÉ?¶­µÔMC?ïþÎ<],?=¯:7zv?#:->?=¯:7zŽ?ïç.$u²B?j`Dn!?hÑۊM½À?j`Dn?ïÿâ†öy·>ãwJ/TÜ6>íy	†Hi>ãwJ/TÛ?4FGL J0348.2+6035?´³ ˆqá@?Fí$[)À:""W:yÀ<H§+R""@!ú»+Ìw?øê`üšò?Ë!¼•?ÈIÕ·3‡?ö
ˆºNE?ü%1uBø"¿Õq7eGœ¿çåaHÌ"¿ë¡h?¯mk¿±"ùF¨Zý¿¾‹$ƒB¿ãēBgƒAGNbcu3FGL J0348.4+6039NVSS J034819+603509?ïàƒ|"ê?r5aðû?oâ|ƒl²?r5aðú?ïêÜçc¤v?yÀ1ЂF?e#œ[ŠI?yÀ1ЂF?ï&oSý?"õÜ-ÀBè?›?²€]?"õÜ-ÀBë?ï£ÏÈ8§ž?wû윢Œ$?‡
ñÖ}?wû윢Œ#4FGL J0348.5-2749¿µóª|h\¢ÀIv†œfÓtÀ8!ײÙÜÀ;¤ÖO,þ@ž4ge¿Í@³¯Yõ>Ü?™9Æö*?°(U3¹
@ÂܱF^‰@ qÛ	¦qï?ۜÞ]	¿Ý s]Dԛ¿ãÏwÁ¶™¿âOðِ¿çs4_Ù'¿ãUOwÅAGNfsrq3FGL J0348.6-2748PKS 0346-27?ïáoñû#¢?®môxÐm\?nÜ]<?®môxÐm]?ïø*&Nƒ?n­¨L?OW§fÅùê?n­¨L?ïÞ¹f…²Ä?t‹¯J!X/?p£L½&ž?t‹¯J!X8?ïÿþ3nª&>¦Ó´Ž>¬É]›Y>¦Ó·Ã4FGL J0348.6-1609?ïÿÌeÄð¯ÀGÐqÞi­CÀ9˜®Eù•À<Lso"
@V0S.ü@¥M–Ãü?² Êzâõ-?¯²1k

?úÆ`¼Ù9Ã@…‹TÝR?ïÿµ¿â'ºí§7è¿æ¬êÿ½ºá¿åО~蝿Þ5xó0䤿ïÿãåîAGNbll3FGL J0348.7-1606PKS 0346-163?ïÿpúd
õ?#š¦»>?à³~¡p½?#š¦»Î?ïþ^Ñ…?Cc•ÛÄå?*òîWž)?Cc•ÛÅ	?ïÚ_Dlg?t_¶‹-ho?rôÐ]ÉÌ,?t_¶‹-hr?ïò™™ÄL{?I"ƒaïŽo?ZÌÌwgÆ?I"ƒaïŽo4FGL J0348.8-0828¿ìŸ9ÿÀFU•:À;ážëèòÀ<Œb¥Æ!@·ÉI	´4@Í6´ÇóI?̲fnžï¿qÁŒ/U‰?©}GÔUd@Ã3ºÂ‰'¿Ê¤©;¿ê'Âó/7%¿ÁüA""´…¿â=OG"=¿ë&Ü"U?x¿ïý—"ãwAGNbcuAT20G J034845-082422?ïìÖùûqF?`lŽÓ<2ó?c)Žº?`lŽÓ<2î?ïöÑ]Òn?wUh.¡m?RxÝD[#ÿ?wUh.¡k?ïS⻬KO?…¤Ó½'??•ƒ¨Šv•÷?…¤Ó½'<?ïëJԀù?RzŠ7JX£?dµ+÷È?RzŠ7JX¡4FGL J0348.8+4610?Ñxjfå±!À¨¬\ý
À:Œ|¦CÌÀ;ã¦êºô]@7Â4moð@SÍÝnÀ?Ü»"¿e=?çcÖ>»@
"x'@	õ¢š¿ß!Ã~ðK¿Üò{}Nà8¿é‹?äœw¿îÂˌZ춿ïΌŠ½]Ä¿ïÿþˆ0»ŠAGNbcuB3 0345+460?¤ƒ?¡Œ7IG`?ÙþÖýX?¡Œ7IG`?åPHðàº?Òy
'Y·q?Õ_oæ>?Òy
'Y·q?ç°˜qF²?µ«yLèÇ?ÑОÏr›?µ«yLèÇ?ßO«_€¾¨?»õ1Ö:È?àX*P? ¬?»õ1Ö:È4FGL J0348.9-4859?îïڈV²ÒÀHÌM©>êÀ;i%ö3ÎdÀ<Ù=x0"F@£Zì4Ç@«ôz¿Ö?ÁýHëC¿µ¡ÙÀ6wœ?óÙ¤ì³òá@6ìÕ*ê9?ïF®€žÐ¿âH†`Կꟴeͺ3¿ØÜ̉°îJ¿ï÷b|×Â?ïÖäH•AGNbcuPKS 0347-491?ïõŸ§&?^	ž¾?UÑèÀ±²ª?^	ž»?ïޝÄzg>?"JÁ%d™Š?p±ÂÌ`K?"JÁ%d™‰?ﶆöŸ?'#âÛ5ÈV?'^BX?Ù?'#âÛ5ÈT?ïäÐù3š?`vß?âÆ?k/ïÌg?`vß?âÆ|4FGL J0349.4-1159?äŒhv{žéÀFÚ$5inYÀ:E†ö(æ©À<R°«#@ öODú?úUPÊï$?Ãþ>ß¹¹u?°'_~ØÕ?ìRjÑ/2@8®©K=k?Ÿd³dÆÔ¿ç\ðû¿åü½€S¢?ÈS™Z.Ÿ¦¿àuïÛŎ¿ÜìCŠ™AGNbll3FGL J0349.2-11581ES 0347-121?ïþ}ˆŸp? ¶£Um?('vÿE? ¶£Um[?ïýւœ¼…?NR½ô=ÔÞ?1KëÖã?NR½ô=Ôé?ïôÕúÝÃ?f؝Jè2?VTÜDzº?f؝Jè-?ïøëujÿ8?<§;/òÂM?LR*T"C?<§;/òÂs4FGL J0349.6+2410¿ëÜbTE}´À7°³''dÀ:·ÔÌuŽøÀ<8.Ýc@°ŸÑ—ö@Þê· ?ÒBh$¬‡³?ÜV܅§tN@KŒ@Ã@	ޖMß²¿äïÍug‹¿ÞÓ0~¢ó5¿ëÙúnƇ¿æ‰Éb4'¥¿ð?ïÿæj,ĄAGNbcuTXS 0346+241?ïù¬$(ö?\ª'5†›?IOŸo\*?\ª'5†"?îø´š—?·A+֏E? "¾FV¥?·A+֏E?î5#ò
¯L?šõÅ~h"¹?¬­ÀßUA?šõÅ~h"¸?ï7ƒXñ?‹Ü3N˜î?™o"ýaÏ?‹Ü3N˜í4FGL J0349.8-2103?æØ£÷~ŒªÀH"tûTŸ•À9€'،À<·ÀÌ
Š@ÐÃAØ@¶øº'`æ?«Û®¢Ñ?ƪ[É)*@Aél?Ä;@w¢jxš?ºËŐÃ\6¿âûMÿm'¿æÊé½ôAÜ¿èÂ:ØC""¿ìd3áƒé¿ïü³µ¥iAGNfsrq3FGL J0349.9-2102PKS 0347-211?ï³uÚ¢!u?¤$1ÃöG?ƒ"‰Ww£9?¤$1ÃöG?ïð`…2¾?(çÒI7?_>õýš†Õ?(çÒI:?îp²çÄ?žN7F#?¨ÿ¾у»?žN7F%?ïñ¹Í3Î?L5]Л?\Œe™üg7?L5]Я4FGL J0350.0+0640?éIèó×ÀA"ãÞaIÇÀ;…BêÊÀ<–'nQí3@#Ç£Œa¢²?ùN"wÉe9?ΝñµaÌ?aoyyWsž?ž]÷íÛÕ?ý—ÁREG¿îb,°b2û¿*Ù>ís¿éTr]•‡f¿Ð$÷0M¦¿ÕÝìd—¯4?Á].Cà)¡AGNbcuNVSS J034957+064126?ïÿy& ?æ32Çî#?PÜ;<+v?æ32Çî¸?ïú¯œ&›¥?^gr…'?EAe'o!?^gr…5?ïë84lÐ?g•@Äã?dÇp˓/ž?g•@Äß?ïï"˜à0C?[ÌS"-^?`Ýgϼ ?[ÌS"-O4FGL J0350.4-5144¿á=B‹ŒàHÀHDââ¸Ç\À;ªœ÷,À<Ç÷øʂ@ Éh»€I<?üªzýÍÙ?Ã:h[´×?ªà#Á¦(?èÛB±Ux@žÞýÑÒp¿îÔ;kç?àÖD°39¿ã&…¥ÆΆ¿Ð¦c"¥¿Ü¤ßÈÒí¿Ú'Z›WûAGNbcu1RXS J035037.0-514457?ïþ¾JëÂ&?ÝCCÃ0ÿ?$QCÝ«E?ÝCCÃ0ú?ïýâ"C‡?VHI‹¼?0ëÝçÓÈ1?VHI‹¼?ïõKµÜ_??]šG?Uh"GA€?]š/?ï÷µd¸`*?Aµî¡?P•6?®@?Aµîœ4FGL J0350.6-3226?êìî‡fÓ%ÀI"ìé¢ÆiÀ;ØÚø»À<ÆEéïƒ@½Õ
8!Ú@ÀRP.ì}?ÑHµüPÈð?Ï¢$Ø|ƒ?ö!‹»Š…*@3I!ßÏ?ï­¾Ña‡¿Ø؄{zIÈ¿ã<6¢(‰a¿å
pᔅ¿çב#'¿ðAGNbcuPKS 0348-326?ïÿchQÁÈ?‡T€IÊ#?'õÇÆð^?‡T€IÊ?ïþŽ=8"@?DE"Jw"?',}Üè?DE"Jw?ï7ê[êœí?ù>ˆÙ?™´'¬bk?ù>ˆÚ?ïÿ~!œÚ?$«Á?<ÛÌdËW?$«ÁŽ‹4FGL J0350.8-2814?äŽYW¡þÀI@Ü­¡À;;y‹YÀ<¤v¾£>^@"ÒB?úkKøüր?Ëv5{âÏn?¨g=beø?ßUŽ7ï@;­$æ¿<¿ïÿm¾Ÿb†?î½µ7"Ñ‹?É®«d_1¿èÀO`c?Ñt¬¥:¿¿ãÎ#¯1±SAGNbll3FGL J0351.0-2816GALEXASC J035051.31-281633.0?ïþ
åw°?9ªã%,É?/!¨ú?9ªã%,Í?ïýډÉ ?V(³NË+¤?1+±·ó1?V(³NË+Ÿ?ﻣî67¨?+ïñT?rr?+ïñU?ïú¹K:ñ?>†5=ÞEv?EÓ¬@û?>†5=ÞE?4FGL J0352.0-2516?âõ·^8CŒÀHÕ³co;!À;R>{fÀ<Å憲6I@}pŠìÙ@"Pi¤ßH?Ó°°!á?·óÔMŸ›?䦸ÁRT@fA'šÇ—?âd"¿éöñL¿çÛBEÈa¿Ïˆâ|·`ª¿èàYTÔ¿ïúÅÞÆõGAGNbcuTXS 0350-253?ï÷òð5Ȉ?O¼Óåí "?P"nò?O¼Óåí 9?ïðEXP*?zu:Ž×
a?_uO_Ū-?zu:Ž×
b?ï®ùÅdŸ?ƒl'ž3"?"AŽ¦Ø?Œ?ƒl'ž3ƒ?ïჸõ'™?[àv^9ñ>?n|G
Øg$?[àv^9ñD4FGL J0352.9-3623?ê¼3Ô`IaÀIYJôðØEÀ:øº˜â›À<uä;~[P@!@iGA]?ôÜZ>9÷s?Ê^Í?äF'?Ó7þ(Š@	™N?Fg@µt«ùm•¿í·4µs¿ë¼=¾&–Ã?æC¼ª R¿Õ‰Ïa§Ñ¿³`#%¿âh'Ü\AGNbll3FGL J0353.0-3622XRS J0353-3623?ïòfôp;4?Z¾«kl;?[2‰™8?Z¾«klA?ïû͐^?[dEaÎ#œ?@Ëž†?[dEaÎ#¥?ï4¨ç.?"Sñ–^/?™jÿþã2?"Sñ–^-?ïñ¿…ÈÒ?SÚ¸¾)Àg?\€ôoîZù?SÚ¸¾)Àr4FGL J0353.0+5654?Ï0ç«®q¥@¸ÌŸóPÀ:ÚH¶RÀ<VÅßrÂ@ jÞ~¥øM@CÂb¿'?ÀŸR–$ïù?µ´"K æ?ó5'éSì@ŒS'Þí¿ëo>&VV?ïå…?ðZñ¿Ø½ây1o¿ß,'Ûç¿ä'è̱¿ä61_žv"AGNbll3FGL J0352.9+5655GB6 J0353+5654?ïúñ\iÂ?Deªt*L?D:®Xú?Deªt*E?ïÑÂ#=¼®? ßêg¨Í'?wîa!¨Ï? ßêg¨Í'?ïáB{¯?uO‹QS¼?n½"Pø÷Ÿ?uO‹QS¸?ïìoù£s?Uˆ Ûgnº?c\Œsf?Uˆ ÛgnÇ4FGL J0353.0-6831?ïôáj-ÀDbŒL˜_À:r)ñkÀ<qä"rÁ@!ñnmpñ°?ú.kßL+?¾n­¡},•?›¹·Ç,#õ?àáP¢"ϳ@ó͞Xñ?ïT{昿Ú{´Á¾%ë¿â'OÐø«x¿ÑĪ¿[Ë¿Øše¼Tº?•©˜5ÁXAGNbll3FGL J0353.0-6831PKS 0352-686?ïýÓ.ÒÓÙ?0ÍÎÔ6[?1f‰ia?_?0ÍÎÔ6x?ïûf"a?dý©`ø«u?Be¿­®{Û?dý©`ø«r?ïí 7"?nU†¤o?b_åÈçjý?nU†¤d?ïÜa(°«å?b˜"ݸ''?qÏk§ªá?b˜"ݸ'Ž4FGL J0353.7+8257¿ìÈ@"K¼ž@6Q?´‰À;X®í¾µÀ<¿í
´ôi@!Ӑ¸ŸnE?ú"âÀ*'?Á§¦b)ë·?¨¦ÜOKÃ?éÐ_Sw¡@à[\È
¿ë"m‹?ïýä1m`V?චpMoõ?£S=ÏÕ|¿èšˆҜ?·ÊùŸ$QAGNbllWN B0343.1+8247?ïúŒ&V?AùnrÊ?EÏg²§›s?AùnrÈ?ïú‰‹ÌÍ<?] ˆv\˓?EÙÐÌËÆ?] ˆv\ˏ?ï­++"o§?"02þs0?"µ5ä\?"02þs0?ïØh±E6c?iè&˜Áåž?s˧]dÍÑ?iè&˜Áå4FGL J0354.4+4643¿½ÄLK–#À"¬ó±³À9,ó*.§³À;˜ìÿr;‡@@õÜ»'M@*º:#?¶` ¦Õ?¼ÃÎ!`£@§Å¬G@(BÒ¸t%?íQ5aáœh¿âY>?€Éi¿èw
bZé¿äœ¼cÈý4¿ê§l ½$c¿ðAGNbcu3FGL J0354.1+4643B3 0350+465?ïù[/NŒl?E²âDÝU?J"BÅÎN?E²âDÝF?ïú²œEn?cá‰èó&?G'5ŽêP¢?cá‰èó$?ïu›$¥T?ˆiÚ'Ú~?'LŸ{kUœ?ˆiÚ'Ú|?ïÖÓC|ó?^i'YÊé ?t–^AýŸ?^i'YÊé!4FGL J0354.7-1617?áÅFt"‰ÀG)l?Ä;.À:û|üªàêÀ<€ž @I¥Î0O(@×N›n…ð?͆-—¡?³ÓÄ[d*?áº}ibD@"hMò&N?â"õbîâ¿áuҟʋ)¿åw©Ÿ¡—¿ç‡¶"v¿ïÿ•Âû?è½hvAGNfsrqPKS 0352-164?ïÿ"‹Øö¤?
ä¯ØG?	ÂW'Q?
ä¯ØFp?ïþ‡c†a¹?CÂþ%iú?'‰Ç™äoT?CÂþ%iÙ?ïâL_–~?q§Õȇ›–?m³÷ i€¾?q§Õȇ›•?ïþoéx€?旣kŽ?)hwÿ™x?旣k4FGL J0354.7+8009?ª'Öä´?ê@4á?J˜«À:[í£)æÀ<–!à$˜f@vlÉ×Ïà@SR"Ã?ÀL"½ê[Ô?À¦ÿVýé?ûpû€>~Á@tP¬ñT?â­ž´5§?Öë©|Åñ¿ã"_½Õ¹¿åv·'"…¿ä»¢£-—¿ëKf/ßÁœAGNbll3FGL J0354.6+8011S5 0346+80?ïóÄ­-?[år·›Z?Xwü¤ß¤c?[år·›Y?ïûNþr:?Z]ȌuÒ?BĶ7*?Z]ȌuÚ?¡[¹?‡Ÿ…x{…?‰Z©›ó?‡Ÿ…x{?ïÿ¼|+'a>õbžæ»?àõ§°Õ>õbžæ¾$4FGL J0355.1-1841¿Ùß+24ÀGËs2'À;?¦½oÀ<ÇQâJãS@ Êæm²¶?ý6Ó¼)ç?Ñkúú݁P?À!hE
Ñ$?짧¯i?ü¨ÚiÃh¿í(¾ÐŠÇo¿ì	| ºu1¿ÃP"'5ú¹¿ÕEM\T>Ç¿ïхc¯˜?îÉ,«AGNbcuNVSS J035513-184309?ïýÀ¼ØÞ?1™°%áy
?1ÿò9€?1™°%áy?ïïÐR} œ?tÅǨ|Ց?`/­'ßcé?tÅǨ|Ր?ï¦^¿ƒ¢?"Û°	q[?†hP:ŸS?"Û°	qX?ïßH‰ßÐ>?h¯¨a}¸?p[»á‰?h¯¨a}´4FGL J0355.3+3909?좠-U»'À&uš¶ÐÀ;gÐâÜÀ<w´ÃÁ‹P@"­e«£?ü¤
5ãè?ÐáÛý—E?¤l…~	?ÙuJÅK#??áÀÛ'£H¿ïêu¿Ÿ½ ?ïþÒn¥Ð¿ÐœEÛ×V¾¿çšãEµ¿½TfÈ{"¿àÑ(l0AGNbcuCRATES J035515+390907?îœÞqCIÔ?Ê( î?¦2ëËbÉ?Ê( î?ï̱`&$?´À/Y¬¢?¦iÓû;"?´À/Y¬¢?J—?‰w.DÚ?Œ}ºmZP?‰w.DÖ?êÌފ2—D?µ¤‡᳧?Ä̅×5¢ó?µ¤‡᳧4FGL J0356.1-1329¿é`\'y©ÀFq[ÕìÀ;,ÓD¶vÀ<µ}¼Ä@´HÔÛ.?ÿ<r\=îx?Ñi·¿Ža?¼nvÖ 2¥?ëw "~–@a[0RX=¿í€
Fªß<¿¶Ê=ü9÷È¿äüYòŠÌ¿×xXKo¿àKs2&Ä¿ïöÐâC6AGNbcuNVSS J035611-132908?ïÿOmQˆª?¦ÚUâþü?UÎêÁÄ?¦ÚUâþÚ?ïýmq¿·;?UDy.?4"rF,?UDy!?ïêÊÝÑ`?kë…Féq?e5".Ÿí
?kë…Fép÷?ïø×¢Ëå?A.ìœ"æ±?Oì¡tÐj×?A.ìœ"æ¾4FGL J0357.0-4955?Þ¢D7ÀH	‹`ñ²_À:˜WšÀ<žßVø4@]ÁÒî@¯!Áçã?¶Ùã`·û¯?·!ÕgÐô¥?ÿ3;C£@^ÎTsö¿é‹fe¦Ò¿Ñy‰¤*¿âÄãß»¿ã™ã€îR¿âĀÍð¹¿êv›r·®AGNbll3FGL J0357.1-4957PKS 0355-500?ïßUób¡?qh¼NÂBÚ?pU9N®û?qh¼NÂBÙ?ïõb¶â¦Æ?f@Ƨò¯˜?U:':²sá?f@Ƨò¯•?ïw€FÕöi?å'¹.Ë%?'÷%A2Ö?å'¹.Ë)?ï¨
·ãÑ!?ròB0ß?…ü'·å?ròB0à4FGL J0357.2+2320?é`ûC?ìÀ6zÞÑ·À:ŒÄ¤	_$À<Legbå¨@ùþ«@ÿÉ^ƒC?Â8‰‰V*"?¨<S~"j?çسiy@ž'¯jfP?î0A`ó_ß¿ßztÛt/}¿éƒ1èEÏ¿ØӦύ¿ä¸é@ ¦¿ëL°/bAGNbcu3FGL J0357.1+2325MG3 J035721+2319?ïèi"äbY?`[ƒQôg?g–k¦€?`[ƒQôc?ïè²¢¥õE?~³pSãÒe?gM]Z
º÷?~³pSãÒe?ïÍhËZ>ã?vwJL=ð?yKšRàŽ9?vwJL=ç?9µ"?s¤Q#—?–ûq'·¢?s¤Q#˜4FGL J0357.2-0319¿Æ^i‰`´ÀCÖb^™éKÀ:È5A*l»À<]IfË@!›ÖY¾bQ?ú³Qf$!G?Ç×&—ïJ{?Ã
pÖ×½—?ýÅÆHNMk@†¼
Ý©"¿ïÿ^Ê¾¿ïƒƒwï$æ?ïÿ‹Á>Ï¿á§Áåèý…¿Ó¦¶ão+¿Õ,0àr›ÿAGNbcu2MASS J03572609-0317596?ïü'Ùäê?C‰¤ãⶮ??›q0ا?C‰¤ãⶹ?ïýdU—Óæ?TqÆ'ñ¬?4ÝSA`Êô?TqÆ'ñ±?ïâ%õ&ty?p¢²²u?mÚ
ً†¬?p¢²²m?ïêm'°?[€S°e±¨?e÷'ØóO'?[€S°e±³4FGL J0357.6-4625¿âT¯•ûÌÀHd\6fÀ:äÜüŸÜÀ<Ò´%t@ô¦›µ¨™@³'[·¶»?"xŠ«?3?®ªc°y?ëGæ^d%@#®ýY¬?ïíZPü¿ÙúsCn"³¿ä³R"ÿÝ~¼¨š¿é"a å¿ïÝDuAGNbcuPKS 0355-465?ïî/KSÏi?]Dµ'h?aд¬0–K?]Dµ'h?ïû <"ž+?W|¡ÿ5g?Au‡Q­?W|¡ÿ5j?ï­è‹…‰â?"›avðµ?"…ݝ‡‰?"›avð³?ïÛÑ«±ù	?^†:©=í?r*'|?^†:©=æ4FGL J0358.0-6946?ÜÈêMê³ÀCÛá2µ^òÀ<'³1fªÀ=Šlê&3@˜<%u/'@|x £?Ý}Œó˜ép?ï>ž¦Ÿ@ÍýAÞÌ@…*ÁõƒO¿êÝSb}£š¿Ûí¼[t'?–"MWÕ1©¿ã³_¿-R¿ïüz¿ï—7z>ŠAGNbcu3FGL J0356.3-6948PMN J0357-6948?ë3OUV×?Ätܚ	Ð?÷2ª¤¥?Ätܚ	Ð?êz¥òÖzG?΁׬?Æh4¦å?΁׬?æõ¿£‹ê?³Ú}büƒ?ҁ޸è,?³Ú}bü"?ÝÛ84FŠ?¾+¹Ò?ácåôÜ»?¾+¹Ò4FGL J0358.1-5954¿Û	Uwé–ÀF=žbV6mÀ:ëIBi1À<Ïs]Å­õ@oéò¢t@¿Š:›?Éç<t$•?ÁŒwG4G?ñíÏ`ûÃZ@oûe'?ïýfȋõl¿åÍEbàŸè¿â˓¿å­÷¯î¿ëÒEb	àT¿ïÿôw5ÁƒAGNbllAT20G J035814-595233?ïî×èó²?t&ˆÀ¢p?a(Mðª?t&ˆÀ¢s?ïìÔÁ0)¯?'mMÕ,kó?c+>ÏÖQx?'mMÕ,kò?ï`ƒ4•á?ŽDB<—§?"ï™m]CÌ?ŽDB<—©?ï'$÷v1§?sñ'ü'e?‹¶Â"s–)?sñ'ü'f4FGL J0358.6+0634?ÝÆ]ÝDÀ@Èك"t—À:6
fðÏáÀ<
$ÜX[@ê+‹p@¨÷ÛnP?Ç.ìË?É1‹þ¦c¬@¯/:€.@‰!.-?åkì O+¿Ó9€TN6¿é°"òsP¿âü^pпïÿþˆ0»Š?ïòF~"…‰AGNbcu3FGL J0358.7+0633PMN J0358+0629?ï؏і¿¤?s:rúDö|?s¸4 -È?s:rúDö}?ïýmþËá}?OªB ^?4	 ôv?OªB ^†?íËè@)H? ¤±jcß?±§È½þµ¼? ¤±jcß?ïöªWáè|?D瀚Pœ?R«P</s?D瀚P'4FGL J0358.7+7649?àuxþw­@1Å÷@=ݱÀ:ɬQ,B~À<¡ ÔƖ@c/p0?ýÑÍ¢µ¢?Êm®Ú˜A?Òc¢ýe?þÆIàô¡þ?ïv%5;¦¿éÔMdº¿â£˜@S,M¿Í5AU_ØÙ¿â-sk1§B¿ê:êýdo@¿á—}à€ˆÑAGNbcu3FGL J0359.7+7649WN B0351.8+7640?ï|҆s%"?—	.Î֝#?e¯1›[«?—	.Î֝#?çBÿÂ!'?Ð<*&þÖÀ?Ðßz{¼Þ?Ð<*&þÖÀ?ë×9µŸ½k?¦µc̩α?À£)
S?¦µc̩γ?äËÅ΂C?´˜j.î?ÖiÎtbûz?´˜j.î4FGL J0358.9+6004?ﴅtÌ?@°ºë#À9§)£gxµÀ;®êÏS)@X¥¨¼@}ïAkÛ?ÀG3å?ÄÒU7iù™@(
%ïû@Êú~5åë?ïõâlvK¿Ýˬ&w
¿êãÁ¦(U¿à‡‡émíC¿ïòÄBº³?îI"~Q¿AGNfsrq3FGL J0358.8+6002TXS 0354+599?ïñKlÜné?dׄ/»N?]i&G",¤?dׄ/»M?ïø½€A#?m^͙ʇ(?Mþûr$?m^͙ʇ'?í'ÄME<¦?¤)ļ²Ý?³iݕÖÌ?¤)ļ²Ü?ïù†ù…{?@ÁyT†?Iäê½
?@ÁyTs4FGL J0359.0-3053¿í;'kÀHŒ¦ YŸÀ:ÖêedçÀ<«nñOc@ GʏÜ?ý¶¡è´?Ã,hÿ?³	ÊÀ>Z??ñ…Žd²1@@ó|ç‡8C¿ïþyzϪ?ïöþ~ö€$¿æ";ßT8ç¿Ó0êÄ.™¿á7u‰Ââ¿ØKéBNY)AGNbllNVSS J035856-305446?ïÿ¦û¼¦d?ÞõŠû4ñ?AÖgƒ^?ÞõŠû5H?ïýÑ֝?FÓQOÂñ?1qK{ƒ?FÓQOÂô?ïöbӍ'è?SrvÀØ?d?S:XäÜ1t?SrvÀØ?K?ïù£V6¿i?;ù"<h¡l?Ir§%]•?;ù"<h¡•4FGL J0359.4-0236¿á·>s!ÀCk=ÀTïFÀ;	3Ê1çÚÀ<gjÜì¬@!z²Us¥?úûÏÔ¿	–?Ñb{ö£ð?Éë~:R?üf\Ukl`@¡:ãUÐ?ïvé¡éÜ¿ïÿYM»?ïÿ¦=ìʙ¿ä|{±QFD¿Ãt0é×ʂ¿èèß½jY:AGNbcuNVSS J035923-023501?ï÷?ÏýÎ?RÏ
–šY¨?Q€aücÎ?RÏ
–šY©?ïúÒ	e?o&埡j?D·Û‹²k™?o&埡j?ïe¯ÇCg?Ýø¿ö?"JŽ?Ýø¿÷?ïÌ/…Ú0÷?r¤ß¼QSº?yè=ç"}?r¤ß¼QSº4FGL J0359.4-2616¿ï"«-ûUSÀH>›A:À:¯8lÄNÀ<k5îÏV@"÷Ô7z@@J@Ejm\?ńüéõýs?¡ˆ6ð¬ûÌ?Ù¦:ý,)@++àÖð?ë:kkˆå¿ãó$Oj¡_¿å··6¿àŽ4á‰t¿Üõ¡'FA¿ïïуjƒAGNbll3FGL J0359.3-2612PKS 0357-264?ïòQøßÄ?Q¯¡/Ù?[\@wɳ?Q¯¡/Ó?ïûÂ*'ª?Z8¢§b›^?CÜ÷UµX?Z8¢§b›b?ïØ£€…tÏ?r9Œ×Y?s®?½E˜%?r9Œ×Xþ?ïàâãÏD?\«Xãm?o0ð¼?\«Xãq4FGL J0359.6+5057?í†2±µx¿ùqé¼ÇœÀ8$
!¼À;.•>Á@hDn
B@ÊâçÁE?§Hÿh^?¿×­?W@E™›@"Ÿe‹u¿Û­øᨦþ¿ãwµxó0å¿çlÜ×ÜËH¿éw>û¾R¿ìƓͧ¾¿ïÿ¸SåZAGNfsrqNRAO 150?ïüI­ÁF?<b_üè»È?=²'õÏáê?<b_ü軾?ïæà—êÔL?"¸bc
=?ih+´d?"¸bc
=?ï^þ³"ò?"FAH£Má?œ´ )a×?"FAH£Mà?ïýGög«%?*GÌ[-W?5ÀL¦àú?*GÌ[-J4FGL J0400.7+3920?ڗ̍›kÀ$o"5ÒIäÀ:-idÒÀ;£J@·?ñ\¤@н¨"?ÉӎG€ó?ÓãùŒ|{?öWþ>^à`@&èãÙ®³?]ʶr¿Ó;Z^›@ä¿Õ9ÐfqN¿æ`MÈá¿êÔ­kÞul¿æ¹£Ÿ×Ì/AGNbcuGB6 J0400+3921?Ù!Ç<?ʳ—•[¿_?ãzsøoa?ʳ—•[¿_?îÄr†2q?»4">7n?¯"¸×œÙ?»4">7o?ááZò'Ô?µVÕ&€#?Ü=JûàW?µVÕ&€"?ç?'™Ãº»?²Ž¤—–ÿ?рúÌxŠŠ?²Ž¤—–ÿ4FGL J0401.0-5353?ïÂdʏ%ÀG*UC(s½À;NXø¿™ÞÀ<Ïq¾‰=@!í\MÞ°$?ùr_µj?ʏ˥†Í?°Io	Î
?晐?'Þ@ƒtük¡?ï×£ -²k¿äRW…øÒå¿âW˜" ;_¿ÖÐ5'BåÙ¿»F@V1dý¿Ó5½|!åAGNbcu3FGL J0401.0-53591RXS J040111.9-535456?ïÿ²`Àг?Tì
Ù??gÏËÓ	Ã?Tì
Ù? ?ïý};RÄ?O‡›iŽÁ¨?4%ißnX?O‡›iŽÁ‹?ïøI
"c,?HNTÞfJ"?NÛÕ²sPƒ?HNTÞfIó?ïø Y­?Eø‡ö»É?OÝâ™E?Eø‡ö»Ä4FGL J0401.3+0412¿è­'pÝÀA?Ú@RÖgÀ:>¥¸‹Í(À<
ïGK@7A"@±¤RZ@?Ãq·<íœ%?§cm1µQ?åujæ'è@y&
«ª"?ïÿµÂÅ¿éæ)«0ñ¿æq´]j>b¿àïÔ;V¿è°a&‹…¿ï÷¡Œ­"
AGNbcuMG1 J040119+0412?ïði¿Åø#?aY¦1yê;?_,€t¸ú?aY¦1yê6?ïù¸Ü´‰¨?^_RžÙ?I-Ù]°?^_Ržî?ïCKiB ?–µdq?·?—–ò׬?–µdq?¶?ïÃà%jtò?i]VNNƒ?~íJŇ|?i]VNN…4FGL J0401.7+2112¿Íñ-ؓÌÎÀ7?uÙ ð¦À9"a#0†±À<ä)à¤@ŽzÒ.5@G6¥®zÒ?±a¹ƒnßÝ?™";$³Ž?äêׯ~Þ,@9¤=Œ}|?¢0ž@¥ë¿ås´È¿çb P‡Ø¿ä¥U~Ž¿å°ÉaÕ¿á=u¬T‡AAGNfsrq3FGL J0401.4+2109TXS 0358+210?ïþ"¸?$Eê­¥?.Î_Ԅ??$Eê­°?ïþƒèÁÿ'?DL+Íé
?'ÁsàÓJ?DL+Íé!?ïëw}8	Q?b:‹˜Å	?dˆ'Çö¯»?b:‹˜Å!?ïÿºÅ[b[>õQÉ îâ/?N©'i¾>õQÉ îã­4FGL J0401.9-2034?Ç{YÏaÀG3'äKoÀ9Žn™:Ï	À<]ʹÍÈ@UBø";@'<O;§v?¯Ïbpãm?¬© Øà?úð¥)œ±@1ûЛc?ïîíôdÁK¿â*^x[[¿ãµo¸õs¿ãa.A?e¿ê\w?&±p¿æ=¨6ëN˜AGNbcuPMN J0401-2034?ïýA*h1?0û©š%Ü»?5÷V¬¾?0û©š%ܵ?ïþK¹¾Aˆ?H¾äÿD‡d?+Ddç}É?H¾äÿD‡Q?ïÁ…†"ts?~à™Â†ø?=<îÅÆC?~à™Â†ó?ïÿS|Sö±?5̌ž¶,?u)ÑÜ?5̌ž¶ý4FGL J0402.0-2616¿ïþ¯9?Á*ÀG׍÷¤ç«À:'C‹p+À<4–åŠ2ô@•§vQ?ÿëî€{»b?»§•/Ҁ–?ÅÒ.
ªRú@
«Ý3L]§@†Êk°??âk6¯Æ,?'‰ÇПÑR¿ßˋ¤cw¿á‡Öޞ†h¿ãxUFƒr¿ïûþ~ÀAGNbll3FGL J0402.1-2618PKS 0359-264?ïäVûÆ*y?jP)-Ji?k©9Շ?jP)-Jf?ïúP})J?]´µ—@?F¾¯ZÖ(?]´µ—@?îêsü˜½?˜¢kºq0?¡XÀ6t.Û?˜¢kºq2?ïÁk'`b.?i™ÂtŒ?J>ÏÎé"?i™Ât†4FGL J0402.0+2737¿ï¦ný‹…oÀ2¦•BCÀ;yD|	À<[Òç™í@¶†ƒ<`@`Ù¼ŸX?Ê(y›ÍP€?¡Ìud8#?ÚÛÏÊ@ÃŒÜÇÂ?îÏËOKE¿äùˆaãÊÀ¿é.f f¿å+§'i?‰ÄÔcw§4¿è…#ÀÏhˆAGNbcu87GB 035856.9+272842?ïüҞãR?5Zž²Å«?9ãkåg÷?5Zž²Ÿ?ïþThî§Ø?Fz›HGÊ(?*¹q'ˆ8?Fz›HGÊ?ïÚQÐáa@?uo­¾§Mö?r׏O`?uo­¾§Mû?ïûð¥Ì#?9"Pþ ?Cˆ=hÏsÐ?9"Pþ Q4FGL J0402.1-3147?Õ&4'ÅÀHEmã2iàÀ:OŠÞó­À<œ£Žåáq@nf½¤:Ý@D–eÖô?¸q¢"¤¿è¿‹è	û<²õ?Òm˜ŸH°@úþ½_Çf¿Êop»©äÀ¿åƒd£î‡¿æ=E¥ü~k¿àŽ1@¿¸½¿æä"pB]¿ïÿÿ" 5•AGNfsrq3FGL J0401.8-3144PKS 0400-319?ïþD•2=g?%/´ñÞáå?+¶¬Ü)Š?%/´ñÞá"?ïþ$÷óÞ§?G…0Q	|:?-°€ÂŒ±?G…0Q	|A?ïòL,±O)?U,'5jÌ?[g¦a­?U,'5jÄ?ïù)±#«0?<K
£Ç?KY;qS?€?<K
£Ç;4FGL J0402.9+6433¿í±¦OËî@!Ü¢˜E܃À;0uєÀ<Md;é»@!ë×ðÂJh?þZj)i…Ö?ݍ}K…:?¬1ž!'u?¯7Ö°ü6È@œ^;Ÿ"Y?ïûŽ¶çˆ:¿än­Aí
Z¿í~³íQ¿°@ô'âÁ¿Ï^z·¬)¿à¼-BXj$AGNbcuNVSS J040254+643509?ïþ™+ù?+YRá+`ª?&f÷
@S?+YRá+`Ä?ïù†‹^¯M?kNíI-†?Iå҅BÊÛ?kNíI-‹?ïÈ4º{?†FûóyÓz?{å¢öBq"?†FûóyÓt?ïó3‡oH?PU:4ZÖ?Y˜ñ!Ópõ?PU:4ZÓ4FGL J0403.3+2601¿"¨íƒ0À3—®FÏÈ*À:uêe:íÀ<"Š•Ø@—ÿ-ól@D@¡±?Éò–J"³ƒ?ÑÕÍ\>Å8@ÐP_"äN@½¤ܘG?ïþÙY£	…¿ç®yZ^ñ'¿èǰބ°(¿äßS¢"j¿ïÿ÷!	:?áê8ÅCAGNfsrqOF 200?ïAÉ«_¹? yø'À;K?—Æʔ	? yø'À;K?îÓ :Ö?¼î¡g¤¹?¯âÍüR'?¼î¡g¤¹?éÞíD"o?°F%‹Ì£1?ȄK¢íîB?°F%‹Ì£1?í‹Û¸Á°_?OnB'²?³¡"9ò}
?OnB'³4FGL J0403.5-2437?ãè Í§÷ÀG{SÞ¤e¥À:|%«‹3¥À<†:8
3@Fëˆúÿ@^®&˜}?¾x2–«'¶?"Úâ»x3?Ò)["æ^ï@

åÓYü¿ÛÖPē˜N¿ãòT{'W^¿ãn=Mh¿ét÷Ãñ[ø¿ï¼jÿR[?îÔ1°|4.AGNbll3FGL J0403.7-2442TXS 0401-248?ïýµ4>v?4A¡,u'?2V_.\?4A¡,u?ïþÀj#?CÄ?n'‰?.ÿy]̃?CÄ?n'"?ï´ú•ö
;?…*¡Ãäݒ?'ÁZ'}qP?…*¡Ãäݑ?ïýÏ8ÅGœ?'A׀Ž{G?1†9ÕÃå?'A׀Ž|4FGL J0403.9-3605?àí¨_!ÙÀH=ÄڐïÀ7R}hájêÀ;¤eƒèWm@j/™@%Ø{V¸?'»˜¼'…?Áœa_–h@*9AÈ!la@!lð—'=2¿Í`ž—i¿âäZB@Â=¿èt¤Ò²À¿éj šª:Ò¿í@j‰
Ö¿èãD]}¿AGNFSRQ3FGL J0403.9-3604PKS 0402-362?ïÜw6‹1?qP=tNÊ?qüÄdºfÍ?qP=tNÉ?ﴘoiCC?œ ðˆ­]?'Ùä%¯/$?œ ðˆ­]?í®ì¡}"c?¦˂ËÊ?²ˆšôìð?¦˂ËÊ?ïǎß:Y?zÂMîþ?|8÷bÓE?zÂMîþ4FGL J0404.1-1715¿î@¶ÖZÒÀFJ5çB™ÙÀ;CTxþŸÀ<Ì۔ìÝ@ )–ˈÿî?þïÙ\'HC?ËÅPV¯$?«—á€"‡?âTŸ^Õxm?ýQµ§—38?ïË$V ž¿ê‰G;þ³Ð¿Ï¨£¸+€¿áãÚÀ€c=¿ØÄúptb¿ä_@zAGNbcuPMN J0404-1718?ïþçê"V? ?hÙår7?!_7º±º? ?hÙårN?ïøáŒAù+?qøòžÏÉ?LyÎøU'?qøòžÏÉ?ïï7¬â?hBðþ?`óÈSéq?hBðþ-?ïÞu³¹:?]#zÔò?pýÅ&#c;?]#zÔò4FGL J0404.3-1559¿Ñÿ·ï³˜MÀF
–_RuïÀ;O²——aÀ<ÁR¡ƒâ@Žèc¬!Ü@qL"îA'?Ô{Á!Gù>?Ó,Kb~û3?üBkK @$ñ[Í[=?ïëÁ¹É:?Ù-«ŸU›=¿åSç]DZZ¿×õ¡Ø,|¿ïÿúŒ—Ó¿è—Ý÷vÅAGNbcuPMN J0404-1559?ïúgÚ&W?J\ZQêÒ`?Gæ`—f¤g?J\ZQêÒT?ïöí¿èé+?l_OwgS?R$€.-¬T?l_OwgO?îñ]ΛS ?"ÏÂ"3? ê#JÅù?"ÏÂ"3?úäÌD?u´ƒÅ×2?ˆØFÌï<?u´ƒÅ×2!4FGL J0405.6-1308?Ššîñ?¸-ÀEPíÍ9ÚÀ9wdå\æ‹À<KãýjúJ@oâ˜»ù@sÞÚŠ¬?ª»=RÏ¿ŠYE¢Ë?ÛÌӂÉs|@ƒæ2(œ¿Ùʦ¢¿¿äœ´&†'¿éz¡†Íå¿ä9Qàd)¿ïü'¶vI2?ï×i©âAGNfsrq3FGL J0405.5-1307PKS 0403-13?ïÿkŒ˜•n?[^¡s?ŽlíR*\?[^ è?ïþüݚ!y?:+éÝá½? 2&]舴?:+éÝáº?ïÙâW'õI?w+d\GÑ»?sÔ6…\?w+d\GÑÁ?ïÿ˜gm¶e?JcŠÓ>?	æ$'f{Z?JcŠÓ<€4FGL J0406.0-5407?ïÒÞN÷¢2ÀFȒ£"¯À:àŸd´µÀ<±2«M÷@«ó[VèÅ@¯àè@?Å
ÈÂ|?¤Õq¶ü€ï?à_o1CD@?ûH
ZÍ?ïæW¸M¹Ç¿êË
å›Ð«¿ÚƒÊE‰ø¿ãð'~Êá:¿éž%"ôÆç¿ïÿý±q&´AGNbcuSUMSS J040608-540445?ïú´_ã.?L2SèÁä?G±.€sI¥?L2SèÁþ?ïúÎra,?Z/•£æ¤¾?DǦ6{I?Z/•£æ¤Â?ïù;äˆ/?ˆâýO::?Œ±ÝôO?ˆâýO::?ïã4k£?["Î?¯©?lë˔\ü0?["Î?¯­4FGL J0407.0-3826¿êáž|hÀGð:}ªOÊÀ8'pûëžIÀ;ÌÊ÷à@ÊÊÁ¯¸?@øfC*÷û?£w£%o·?¼¨ËæÙD@ÿE™›@Y؍Ë/>?èP«Hî†[¿ÝJŒL˜_¿åÏÞú÷­¿æ^ä&…¥Ç¿é!(n´¿ïþ'jöîßAGNfsrq3FGL J0407.1-3825PKS 0405-385?ïøÃ|€‰÷?K"ºêzµ¯?Lò
ýØ#u?K"ºêzµ?ïðªÈÆ?€;ž£~}?_öªnt??€;ž£~~?ï'ÒäƒCˆ?ˆIÇýé?‹KFß/#?ˆIÇýå?ïôú'ÍÔ=?J
¿zâ?V°dWß?J
¿zê4FGL J0407.5+0741¿»÷¦	0]À?$GäÀ9U¸éÀùZÀ;ëŽÑ¿zÕ@Ç=ûc84@Wn{ޝ°?°Øú''–ñ?£(:[ÆzM?òqV8ú@½Œqg÷5?î 'ódK¿Òý¼-î%¿æºUÑ쓿ä5ëß·‹¿âû"ÀĀο倴%6nAGNbll3FGL J0407.5+0740TXS 0404+075?ïöLñÚv?Jz\Pi`¹?SfKût?Jz\Pi`¦?ïþ$]†®¾?Jñ!Ê÷Ö?-º'•/V?Jñ!Ê÷¾?ïË3
þú=?zJžÉÞ?zfz€'áÏ?zJžÉÝ?ïêx?SbGŠ%»?eéô‡éåB?SbGŠ%Î4FGL J0409.4+3201?Ñ­¬¥ž¶À,»"F™A…À:j«¾_KÀÀ<L)'ÉÁ€@ aùkç.Î@XKä ÷?»`¥_?¬¿n!¤H&é?Ö`½Z?ôÁ­]è?ìw~¼ž¿ééKRä©b¿àA|lb(ê¿Ó†_!£"¿à`¯"#¿æ'z-ǪAGNbcu3FGL J0409.4+3158NVSS J040928+320245?ïî©æS|ˆ?_ßu{n?aV¬ƒwÄ?_ßu{n?︩α›}?—x©gçž?ÕŒS™ ?—x©gçž?ïà—gʜ2?t
Á¤üÑw?oh˜5cΧ?t
Á¤üÑ{?öm?ŠÝv¥ÚOB?§·?ŸÙJ?ŠÝv¥ÚOD4FGL J0409.8-0359?܌"A³°ÀB°€Ç:¼"À:0î'hÀ<K.cÀ™¹@¯'aÁæë?úօ˜ZÕ9?ºê!Fv²?ÓÛgšC
@ý+¿¡k@ö0툯?ï—ÆZÂÄ5¿Öµžþ'U¿Ë"Îš¿ßW
:M"¿ç6Ë£×àý¿ì+½óëõ‡AGNbll3FGL J0409.8-0358NVSS J040946-040003?ïev~?'I&±"i?"Q0=¼_?'I&±"i?ïöHfP'	?iVáò7ZY?So3^ûë"?iVáò7ZT?ègVôÄÎ?³ûk›p™?ÏÒb¤,ìÅ?³ûk›p™?ᆵyò¾>?he[/¥÷6?€T!ƒPp£?he[/¥÷=4FGL J0410.9+4216?ê·f»7ŽÀ&Üã›EÀ9t»=¤¦À;é?l&š@vI±ú¹o@ËN˜‡œ?¶®#ÿ¹‰#?½ÞúaZë@î"þ"?@X1` (Õ?ïµK;gµ¿Ÿ¤,€Í¬¿â<à<Z¿âÊ|ûÔ!U¿â¥É㽿맾ŠßÂAGNbcuB3 0407+421?ïôÄuäÿ?Wîo_À?Vw7ò`?Wîo_Å?ïøÇ,†$'?e£ÜՊP?LãMçmö:?e£ÜՊN?ï¯{ƒÁxg?pJpN¼?"!¡æ%?pJpN¶?ïÈkÕ¬9²?dðZ«dó¾?{Ê)ã'6?dðZ«dó»4FGL J0411.7+3041¿ëöÇ{¯ZÏÀ-ó—»s5À:ÃÑðøüÀ<#AՍe¯@mqÕ‹@pÈ¥ߙ?օÞzt:?慍Þzt@oçáüú?þä#›e¡š?ïäÊ"%¼?´'ÿ¡‹U‰¿áˆÞ@<±¿éÆh¸P>¿ïÿ}#AM¨?ïû?!ÎAGNbcuGB6 J0411+3040?é•ï¦ªN?Æ»Hœ®"T?ɨAeWâÆ?Æ»Hœ®"T?â[äBà;?Õ	/<*ä?ÛIæ7z?‰?Õ	/<*ä?äO¢RÒ©?µj¾ãáh?×`»Z[Ü­?µj¾ãáh?ÆÊ֓!9d?²¤vB ì?êMJ[7±¨?²¤vB ì4FGL J0412.3+0239?àŸv…°‹³À@™3]$žEÀ:4±‰zg¥À<³˜H`Â@r_˜ìË@b%#¥÷v?ÁZÌ)cь?®@Ÿb4?î"ЧLàƒ@3U#‡¿ã¿9+
Ë?Òµ)­xs¯¿äâ~—_®¿ã Þ҈Îp¿êŠDý`¿Þy–ÄÓHAGNbcuPKS 0409+025?况kÕìe?…ƒüÁ¡i?…"¥
"æë?…ƒüÁ¡k?ïý¨œ¤ù?Vi—YGÚ+?7ò»Ø4o?Vi—YGÚ'?ï$,Ä©?"'If?›z|ÇŠÝ?"'Ie?ï×P˜Œþ?c‡i{_óe?t}W³¹€;?c‡i{_ói4FGL J0413.1-5332?ݔЄ3,(ÀF\Ïkã}éÀ:‹…ÛÀ<QäJ—ÓÇ@±Šû"@/«SÖ@ê?µ¨Á?O÷?—°þ‡|X
?á`fQÒ@Ußêáµ½?ïÒéçÆ²¿âIfÿQ"¿çVSÉ«°¿åH¦4¿è|z¤áÌ¿Ý·Oµò–AGNfsrq3FGL J0413.6-5334PMN J0413-5332?ïþjÏ7—Ú?%Oð(vMÙ?)S†'Ul?%Oð(vM³?ïþyû<q0?IAqÔ]«?(`L8íù?IAqÔ]«|?ïë¬ðMBá?b_'MÕ»Î?dS²½V?b_'MÕ»È?ïÿâùVhd>áÇ£&lÜ>í©—›i>áÇ£&j^4FGL J0414.6-0842?æς^«ŸÀCW¼]éÀ#À;W‹àsr¾À<§ü­e(y@àoW%Ö©@æ—b%?Ç鮄ã)0¿…/n=Üj¶?¿a@Œ¸	Ç@›2֖û?î©z¸-˜¿í;ž§"?'n6'ž¿æ¼ˆabñg¿âÙA…Þ¿ÔíUBý€ŸAGNbcu3FGL J0414.9-0840NVSS J041433-084206?ïýé굞Å?+4ΰµ?0°ªS	Ò?+4ΰƒ?ïþ£ª\ÑB?B6vՄ–?%ÅZ2ëÏi?B6vՄ–"?ïéŠÒ1¥-?r@²QH(a?fu-ÎZÒ~?r@²QH(]?ïûË	Ô;‹?0é}jéo?@ÓدÑþ?0é}jé^4FGL J0414.8-5338?ßñ»!윛ÀF9Ç͉‹/À:ß´tç2ªÀ<ŒZ{v™@!Æ.Ü"?ú¿$º|?Él;½pc?Âu	ÂK"~?÷Dî|Iýz@¾ØR'ó2?îQí}ÇV?×/!°ÿ½¿ÃW—ULj¿Õ]ä·¥¿Â®9#b/Ë¿èg²GcAGNbcuRBS 0526?ïôΔ‹\²?R'lí_G?VbÖéFšS?R'lí_A?ïùïuoÓÊ?j"VŽ•?HB*@°Ôè?j"VŽ?ïáirm	ñ?rõ²Àx¼?n–'ö¢?rõ²Àx¼?ﲦ§gZ?t	ˆ¥á¤ö?ƒVV;&)¨?t	ˆ¥á¤ö4FGL J0415.2-5741¿ÙošÑ_XÀEŸaܓê-À<1 'EÀÀ=Gýœ@#`ãÍDkë?¤=Æ_u;?ä':l˜•?ïüšò?ÿÛÄ?þ©úE+¿ïþæ?d™Þ?î¹NjÇ7¿Ë©nù²Þå¿ç8Ð@Ô?¤0Q<Ľ›?Å¿ˆÁ…AGNbcu1RXS J041505.7-574237?ﯵ«lÁ4?…
ŠÔóã/?"•$ϲñ?…
ŠÔóã.?ïùˆ‡"±Ô?lÅìúÚ¤£?IÝá±8±½?lÅìúÚ¤ª?íÈIˆì-? âٞ³¿-?±½·K¸ž™? âٞ³¿-?ïì¾_†ã?j@¾Þ;¬Ž?cA yë`?j@¾Þ;¬4FGL J0416.0-4743¿ï´|½ÀF½#N¹¡wÀ;fÞõÄ<ÛÀ<ßùË2˜Ú@Nšþsì@xä$Ø&?Ò-úNw\?Ë!É(}w¥?ø[Ƶ[—@(¦h´õ@?ïù–Ys8ݿތ¨ðN²¿ç›Ê`áÂ'¿á±§­Y¿ïÿ¯Èe_¿ëý€Ú†AGNbcuPMN J0415-4737?ïþÉßÁÁ?7åù"½Ž?.óbã×?7åù"½‰?ïúÐN`?c95pÝêY?GľǮŸ?c95pÝê_?ï
~D\
?'1ÛÖéW?ž°7lT~¤?'1ÛÖéT?ïà™gÁ'¹?\ªÂ¸3Aæ?of˜>ØG£?\ªÂ¸3AÝ4FGL J0416.0-6628¿ëœåÁàÀCí½Q.ƽÀ;C¤as¸À<»ŸÖÊ|@òs\æ`@Gý'w>%?Â;…èí¿«£~€Ž†?ëIA'¼Á@º•'LC%?ï–T€4éñ¢Íõ¿硑J?¿3¿Ý½"ÅÌþK¿â&¦'¦`Q¿Ô´AGNbcuPMN J0416-6629?ïûOTN?=@"$Hû?B¯†ÇɄ?=@"$Hü?ïý§"—P?G"¦¢
ë?2ÃÛC}Š?G"¦¢
ò?ïçHêKðÎ?tΨMq?h·´2z?tΨMo?ïò Ýxò?JT|Šts>?[¾EþW?JT|ŠtsH4FGL J0416.2-4353¿âďÿ¼ÀFðîcŠ	À:ßÇÏ7
XÀ<žÑ0ߛÜ@rØòõÖ[@Ð<eáÜ)?ÆH3
‡¶?¿pQ¡³C?óÖރ®uÊ@a"²VÔοïÿÃ.¾Ym?ïþ­ŸàÛx¿æQìAZ¿ë3^ ò"Ü¿ç"¢^º¡¿ïÿס<%JAGNfsrq3FGL J0415.7-4351SUMSS J041613-435057?ïÿ7ꖴm? ù;Ï`º€?­)rS=? ù;Ï`º'?ïýÑà(××?LJBÓÐ-?1pþ¹AFÜ?LJBÓÐ%?îú,æä£?–Ï/n…ü? ]1'¾EÓ?–Ï/n…ý?ïù"'؈B?@2Â!97®?IíôÞú¶?@2Â!97¦4FGL J0416.5-1852?è'ù2õkíÀE3§Å¬À9wc(ÄDhÀ<[²h!@†Ì<Ùû	@ö Ä0F?«ˆ>®ïö?¢ä,å¼1õ?óõãFŒ@Ge€¸L7?Ã_چç¿ãuÒêóÿ¿æ"	\ ¿æ'ä¾®&¿â‡vfœí¿åm¹ Èw~AGNfsrq3FGL J0416.6-1850PKS 0414-189?ïþåAzød?´/$kr•?!«èPy¯l?´/$kr»?ïþkݔ'?H‰™°!®c?)B&¾Ýmä?H‰™°!®S?ï@ ?b)ވ0‹?azÿ¿ß´?b)ވ0|?ïÿÐכ >팮ËÅÖ©>÷"2rï¹û>팮ËÅÙÿ4FGL J0416.9+0105¿ït—Ò_kÀ@"¢ƒM&úÀ9¦¾r–öQÀ<	¹07Ö0@ rÞÎ,j?þ4rHø"?±en™»¨b¿†:A"ÖJ?×]_A. @		l¥Å¡à¿ÛüÑö®H¿ä¸u\£o¿âkIYæ%c¿Õ՞Bà¿áÔM"ÞHö¿Ë¢‰pîUAGNbll3FGL J0416.8+01041ES 0414+009?ïþÒñ ÀK?ÿºÞ!NØ?"ÐíóûMê?ÿºÞ!N)?ïþ?gª"?J$ž'Jú?,	…VÎ\?J$ž'Jú?ï÷òEù™f?W‰ÁÉ2T?PtÍ0‰?W‰ÁÉ2Tª?ïûííô†v?2v"`/Á?@HH-æ$F?2v"`/¸4FGL J0418.1-0252?Ò¥†ÞÛ`HÀA…
¢q›À9Áíûñ}†À;ùôñ¯e@FÔ¸~Œ"@(N?þó'?¹5T`)‹j?ÈOFúTv@
d8Š‹	@™—‹wlô?ïÿ >ybm¿á¥ø¸
"'¿ãm9ßtÅ$¿ãéíÚcŽE¿ìo>±ìv¶¿ïþ–]úÝAGNbcu3FGL J0418.0-0251PKS B0415-029?ïæÛ÷G`?m?põº?i$帞Ý?m?põ·?ïûhöÌR?W`.΁°?B_¤$η¤?W`.΁·?ëjòh"²?«_ÓÅKFÛ?ÂT6_å±:?«_ÓÅKFÛ?ïùy?:?9t<·î?Iú—?9t<·îW4FGL J0418.2+3807¿ÉL,§lÑÀ!ˆr)é–À8ôÅÕaÆÄÀ;mW…!@þ®ð}@ä_á'p?µæÈÌbÏ?Ã11{M(R@SƒãNïQ@
j‡ðú©¿Ó7ØßT¹Á¿äÒ3ß*b¿é¡ÝÀý¿è>°	G§^¿ëØÔ½‡	Ÿ¿ïüøÿZ¾'AGNrdg3FGL J0418.5+3813c3C 111?ïêðÏÂãf?c"Df°?e0=™?c"Df³?ïð
,Є	?x'aPy?_å¦^÷î~?x'aPy?îí˜{¢˜¤?—än*\Ϟ?¡&xEÖuÓ?—än*\ϟ?vƒ?t!//_?‹byŸžÜ?t!//a4FGL J0418.4+3414?ß¿"¢ƒÐºÀ&õû"‰µ À:¶XÆj²üÀ<-+œeü´@¥4°¶Áž@yõÅšç?Ò»ua€ùe?Ê¡õHAe?ö	Œ³?ó9
}‡jB¿Ã>ü•t¿íà
¹(*¿´ZŽýðlu¿àÚ&½+.¿ïÿÜßi‡ƒ?å;
óÊAGNbcu3FGL J0418.2+3412GB6 J0418+3411?ÆÎn?Ö
qì×Ë?‰xŒd¤?Ö
qì×Ë?îÏ»q÷ ?°4ƈ"Ù?£tHà†?°4ƈ"Ù?ìh¬"T!?¦ãMÓ?¼ºží_võ?¦ãMÓ?ìҞpÎp?¥Ú'óY?¹kyŒÈ?¥Ú'óY4FGL J0420.0+0805¿î)ǀø½"À<sz€Ïž8À:¬[y£Z
À<e|[›1@‹¨ÉR9@rT`ªdÃ?Å}
—³f¿"9r½aÊË?Ê·û–ã\@
Ðδ®rð¿ÝN'}ÁKå¿ã:}¿ÉY%¿ëˆ:̄¨q¿áåuoî¥e¿âàØóK½¿ïÿùµc#¼AGNbcuPMN J0419+0804?ïÿLŒKÉJ?¤ž,©ó?nv†Ö™·?¤ž,©u?ïþ+ g]º?J­}nm ?-MùŠ$]?J­}nm?ïÚÂ/‡•¥?sߢê\1Ä?ržè<5-6?sߢê\1Ë?ïþðhÉ©L?ü8{È=? ùsekI'?ü8{ÈÖ4FGL J0420.2+4012¿ï™iq·
¯Àf'ëØ+À:=k¥jˆ4À<q¾‰=+@!	'Oæ?ýHÊ#¥ ¶?ÃwA)@?¸NÇ~¹ï?ôòôcê‹$@ÒÛðX•?ïë³ýÈî¿ç Çä¡Ö?Ípž"ÀI¿ÞÔna‡"n¿Ú] #÷V
¿à‰äð°AGNbllB3 0416+400?ïú4ø'?F"£Jׯ·?Gã/ ¿0?F"£JׯÌ?ïû¬øº4?\ïCXüP?AL/¸.?\ïCXüG?ïØqy}-9?vEA@n•?sÇCAic†?vEA@n•?ïˆ\zË¥4?yÒ­´S€?èáM²Ó?yÒ­´S€4FGL J0420.3-6016?à$—ôãÀDäÁ¨¬\À:ï¨NhBßÀ<Ҝ¡‹Öb@ãü>Ty@Stÿ†]}?ÀíS*Œˆ¿ŸWÐýD0?ޜš·På@¬ƒ!Ýö@?ïÇËLp¿åvÀ4ü¿å¤)	ä…P¿×",<žìÀ¿Ý@IQë¿á¸I©ƒòAGNbll3FGL J0420.4-60131RXS J042012.8-601446?ïþŸ«ëD¤?Hr,'?&AKµÁÏ?Hr,1?ïþ‡CAG€?C;'x7IS?'‹Ëëˆ?C;'x7Ik?ïû†l¹Õg?E2'š'Ö?AæMªcf?E2'š''?ïûßC²B?-al¼8$?@'ñ6÷ž'?-al¼7È4FGL J0420.3-3745¿~šã*nSÕÀFŸ}At>–À9?q/EÀ<Õ]•@º–rȟl@b:îéW?­6(ÛìOt?¯
nݝn?þr!+û1@ ³0C"ª¿Ù€ÉS›ˆ‡¿â/2ÝøÄ"¿ãêÅX.•¿âIáf6ì¿år{Gžû¿ç¸W)²€ñAGNbcu3FGL J0420.6-3742NVSS J042025-374443?ïþÇ¢(|?ÖU»z&+?#…ÞíxLÃ?ÖU»z&a?ïýCúžˆ¾?LSê¸Í'2?5à+º"?LSê¸Í'O?ïî;[	'?ef@À
/‡?aĀ¤öÚ4?ef@À
/‹?ïýÜ5®«*?$0.¤øO[?1RŠ¦¹À?$0.¤øOA4FGL J0421.0-0752?æjô žÈ~ÀBsUïÝìÀ:š*
ðƒ‹À<*ºè@ä²hG'@äŠ=Ü¡?Èö¤Œ'É?°o炅¬?娑¹ÑG†?ðõž,Á?ïý
Ú7¿æä¶Ê,	¿å §ªÔT¿êƒÈaƒ'½¿×8À¦MÝ¿ïü÷™Ã
AGNbcuPKS 0418-079?ïòu»c:õ?lFÓy€ˆq?[‰9Š?lFÓy€ˆo?î¸
͜?³±ÝtçÔ?¤.?£&B?³±ÝtçÔ?îʣݤñÄ?šÜ,ŠÃBß?£UÂ%°ãº?šÜ,ŠÃBÞ?ìþî›ßî?¤€´ `‹P?¸‹'Á"?¤€´ `‹O4FGL J0422.1-0644?î´–­{³ÀBäâmHÀ8Ïk=e¼À;ØyªæÈ÷@mHS*õL@¬¾9Œ?¦-º<@;ô?´ÿ+Ä©èœ@	†Eÿ¾'@¨=?üoR¿ÒÔÂ$'Q©¿âýÄMc`¿çpÄÜ=ƒ¿ç.³Ý¾n¿éÚ¡oB¿ïÞfÝڑ1AGNfsrq3FGL J0422.1-0642PMN J0422-0643?ïþ@ú0¬?$nœ"ÀTª?+þ\õ9¡?$nœ"ÀTò?ïü®…7Û¯?SÐfM¹?:‹ÖA"{œ?SÐfM¹m?ï¸,é¡»Ò?}]S9'UJ?ôŗ'¶?}]S9'UD?ïÿ²"e:O>ø~ê/i6d?^æ±l_3>ø~ê/i6U4FGL J0422.3+1951?ïÛ=#CÊ$À4œ!ÄuæÀ9òQ~wÕ$À<2¯È@ 5;K/©@m|:
B?¹Ç¿FÒLi?‡ Éû"?ÑÝVlGQ@0fšhÌr?ïÁ¢a¿7¹¿çöÿ.=*¿â Va¶~W¿ÕApx8 ¿çÑ@>ßcӿɤCZÃÆAGNbllMS 0419.3+1943?ïýg²¬?6GZ]Õ©?4ÇjŸ|á?6GZ]ÕÃ?ïýúå[Â?MUr
ÌÌT?0(Õ!ï=?MUr
ÌÌ??ïîò¯Bbs?iX'‰½á?a
P½Ž8?iX'‰½á ?ïóQPƲ?Iω©;Rï?Y]^s؜z?Iω©;Rò4FGL J0422.8+0225¿ïœ'üm*À?.¢ ©XSÀ:?Ã<*RºÀ;óvñÎäÕ@–7t‹m1@
'¼«ì?ÎÍÉaˆ[.?äN.Km@ Êƒ@¬Lfn¿ÌmÆWߦ¿á(qy‹¿ì!yÍKwοïø˜'˜K;¿ìl5恿ï¦Ñ€ìAGNfsrq1FGL J0422.1+0211PKS 0420+022?ÏóՀ?'^´çªx?‰ÓŒ
 r?'^´çªy?èø'ô?ÑA—&ڈØ?ψ»Ü0?ÑA—&ڈØ?çCNØ}/?µV´ù?ÑÇybO¢?µV´ù?çlŽ"Em?¶³ó·c™Z?Ññ&ã»u'?¶³ó·c™Z4FGL J0423.1+2106?æ¶L:eÎzÀ3§ÑEØQeÀ9É2ÄxjuÀ;鞍õ ©@ŽÅ9°zÝ@#¿!é_?»Jm·hŒ†?³ôÓ|vÕ?ùÝÑ6¾Øî?úO–@HÅ¿Ø¥bïڿهã¤)Àn¿çù‹!0Ò0¿ß8÷b¢Œ‡¿å·a¿ðAGNbcuTXS 0420+210?ï' Uç†?z²¼EæL?~¶ïÕ=*?z²¼EæK?î_f™?¶ÛçKªNì?ª	Ÿ¦n>?¶ÛçKªNì?îÆÏ´ÜÄ$?—wáØÔÉl?£"²3½É?—wáØÔÉg?êÉñŒfVº?¨ª ?fæ?ÄØ9Îf¥?¨ª ?fæ4FGL J0423.3-0120?ëð\*½À@>}QÀ8
g†!ÑÀ;Á%ϝb@•,]@ätÙÆ°S?ÆÅÝÖp¡?¶˜W¾òˆb@ôaùð†@uÏ¢<x¿Ó;ž̬¿àO8añ6¹¿å-F¿×ñÄ¿åâ;Ÿh¿çèµ@i&µ¿ìsüPHAGNFSRQ3FGL J0423.2-0119PKS 0420-01?ïýì°Y3)?*{ýQÒS?0š}6f±œ?*{ýQÒRß?ïöœæS?k\Ï3Ԕ½?RÆ3×ÅYÅ?k\Ï3Ԕ»?ïßk©·?r?w¨-?pJp+s£ò?r?w¨/?ïÿpí?×T="ê?âB(
Öº?×T=…/4FGL J0423.9+4150¿ëÊ÷nXŽùÀ‰äÁ¶UÀ8X-'JTÀ;`e':ØC@¯L$›À»?üƒ3á®Ü!?¥–˜Þ2и?»övÿ»·|@Áv¹Ã@¿úQo¤¿Ì«¥'[¿ÚÓ³¼¨†¿Ú²!$袿ÔïÂ',j¿â"n!EÊå¿ãÛG¹ÒõAGNbll3FGL J0423.8+41504C +41.11?ìGY";mm?¸A,h@ò?½Å6î$"–?¸A,h@ò?ÌJà']¤?ÑùN4•VÙ?èíGۘ¨–?ÑùN4•VÙ?ëÒÅ
ë?«©?ÿßj?À·ÜêÈY?«©?ÿßj?и»IÌ1?®œÞ¸¡¶??磢[ç9?®œÞ¸¡¶@4FGL J0424.7+0036?׌)ùGìÀ?ÆñVIÀ8«ü†Î»ºÀ;Ý[o'_@Âqû@JTFŸ?§£aÍ/?¬îÄ$÷J@瀕Ó;@S¬½¿œ¿×Õi>!²¿ÚäÑ@±¡¿ä…péP'¿áäø¨ê¿æFV[Vgì¿æÖlÞ¥'KAGNbll3FGL J0424.7+0035PKS 0422+00?ïû­)œiÂ?<±ø½+M?AKYŽXõ ?<±ø½+?ïüѝGV?T,–05y?9sÍÅU¨?T,–05m?ïÉ°Vuª?¥Ë¾À[ó?{v§ÔÅ+b?¥Ë¾À[î?ïäúš®É?]‹îǕr?keQ6ÿÃ?]‹îǕy4FGL J0424.9-5331¿À¦\mnN\ÀEÓEŒÒÀ9­ß…65FÀ<A»±–^@Ź'Fî@"
f‹OT?±®xßöÜQ?½U&^Iȇ@
ÚXÁb5@×Õ?7"¿—I›ªjø¿ß,>ø8`¿ã+åï¿ã0AFmD¿ê¤E>Îqè¿ïþú|2€†AGNbll3FGL J0425.0-5331PMN J0425-5331?ïú§9±º¶?B¢Ýþ^?Ec9*ð?B¢Ýþf?ïüeÏ6úâ?V"÷,1«C?<цH(ôø?V"÷,1«C?îô‹K'I¸?•D´€~V? ·KFÛd|?•D´€~V?ïùâ(…dR?7ÉÃF!‹W?Hw]ênº?7ÉÃF!‹ 4FGL J0425.3+6319?ïÐrت@#‰ù&ÇêæÀ9ì
±™kÀ< ÌàîÂÁ@!¹ññIƒØ?ý_ñ7n+?º ³iNx3?"êxg«ò?Ø©ßAÄpˆ@ò`gžÊ±¿Ùž´@cóE¿å®Å"T¹¿ç¼=s(¿Ñ÷†^ÔKÇ¿Ó\ž¼n¿ÚæØ;ÀËbAGNbcu3FGL J0425.2+6319NVSS J042524+632005?ïø˜ ‰ÚQ?I®2àø:;?MŸ}ؖÀ€?I®2àø:1?ïú6©
??e‹4ŒË¢O?Gÿ%[מ?e‹4ŒË¢N?ïÑKá_Úg?x8
â!£"?wZPÌÌ?x8
â!£?ïÊë=½>?m¤*ł¥o?zŠay¡`Ý?m¤*ł¥v4FGL J0426.7+6826¿èˆ€ãŸ@*º=ú	FÀ9¹ÏµqfÀ<6¸©õ@!lµàÍ
@˜vƒêÛ¬?³¶ûª0?ª´Áp'ý?÷³{?D@yáSígø?ï÷ó¡Íś¿à³ŸÕý¿åŸ+ÿ¸1Š¿à! Ï¨¿ãPW›ÈH¿æ]4Ž}åAGNbcu3FGL J0426.3+68274C +68.05?ïõc¯$ÿ#?OìO¥¨g?U8¡¶¼µ?OìO¥¨g?ïçh9Mà×?'w‰T¤>é?h—Ʋ(¯?'w‰T¤>é?ïðŸãs?fÚHOþ3?_ñôÀ9Ô?fÚHOþ0?ï…Uïv?uZ×ØÌ$Ô?Žª "}æ?uZ×ØÌ$Ó4FGL J0427.3-3900¿îÖ¡aGØÆÀE÷—$tSÀ8ä01öóÀ;´bTˆîQ@å†Tmj'@¾–ÃüC³?¨Î½š
L?y~þÈ#n?ʽì(2@xS/'
¿ÝՂ}ô!¥¿åÝÓð­|¥¿êœ¾™XV¿ç8®6Ý¿ïüC²\´?ï|.NÇä0AGNbcu3FGL J0427.3-3900PMN J0427-3900?ïÿ;½º?$íkîU=?üH¿+?$íkîU?ïüâ¿îþ´?ZâĒì?8êˆ
bé?ZâĒô?ïfûS{ÌÂ?ùñ@?L[?" •†gŒ?ùñ@?LY?ïü´yŽ?4"(ÕÍç?:_ÏL3ˆˆ?4"(ÕÍÀ4FGL J0428.6-3756¿×¦\šª1BÀEέÙ©TÀ6EXôÛöÀ:©fã@È{zIÈ ?ÿë|Öt+?†Nӑ{׬?´ég,ù³@*Lˆ3?È@ QúÖ `2¿³¢ðŸ(¾¿Ú#¡ZX;*¿â'°âÄ¿áýˆV{7¿åé`F'µ¿è Fý"5AGNbll3FGL J0428.6-3756PKS 0426-380?ïΧv[?|fUVÍ£ú?xò,pÄÒÙ?|fUVÍ£ÿ?ïŽQ*
´?§ß¤s?Œkµ|¾ÓT?§ß¤s?ï+äºQ?—LòØꞻ?šœÃh½•à?—LòØꞺ?ï鵏jÌ?'*ÀHøc?œâÉN¦ˆ?'*ÀHøb4FGL J0428.7-5003?ï<)s+*6ÀE‡0HAÀ;O¥^ɹóÀ<ˍg\/¬@í
¡~?v@"!4x®?Î×^v-í?¼/'(áö?îŠÒŒ)nŽ?ô†ùç71E?ïþ±ëÕ¿Ò''Û'‡¿èˆ¥@ï«¿ß'£G˜E¿ïÿŽñ ¿îxê݃ÿ)AGNbcuPMN J0428-5005?ïý±`Ñx?:=­€oA?2wÔùt=—?:=­€o8?îÕzòyx?³'YŽ Œü?¢®XPØhƒ?³'YŽ Œü?ïÄN‰ü?'CŒ×)ß4?üÇv.Àe?'CŒ×)ß4?ì–;óšÀÌ?¦ýŽá˜å?»N c)ù©?¦ýŽá˜å4FGL J0429.3-3238?áh$îbkŽÀEzšu%FÀ;G\WìÀ<иãá¼H@P¦?p?ý™¨bŠ8Ô?ÏN×(›T°?Éó˜Ôw¼?ö1ƒ/ÊÉ@_u†iç¿ïü.ÿò¾ú?ïÿërªAˆ¿Ú#|"jÞ¿åÀ¾/@¿ÒéûF\Û£¿é*°bˆá;AGNbllNVSS J042900-323638?ï÷¬zÞú‹?M‰o¤HÏ?P§
B
éu?M‰o¤HÍ?ïö—ч"?pâLš5?RÐ\ð×Ò]?pâLš5?ï…4ê=?'üŽ%[Ø?ï^b¸j?'üŽ%[Ú?ïË¢L؄»?ma•M7ø?z.ٓ½¢¿?ma•M7û4FGL J0429.3-4326¿ï¾û¥†ªÀEÅõ@‰]À;å(
eCÀ<¶ýwÞ@bå®pg@ýø8‹?Åê•_£(º?¨ "ûé¬?àÿG¾…ŒF@:~6Ë¿Ú&Gݏ<É?¡9À–¾»¿å§ûâd
Ç¿ìSå1[¿âWÝó»¤?º‹¤ùÜAGNfsrqPKS 0427-435?ïúu`ñX?CfÞæ›MÀ?F*|:Ÿä\?CfÞæ›MÊ?ïüßSÌ7¹?]b¨"¢¡‡?9ažB8?]b¨"¢¡†?ïˆco™8?ˆjb­¦?ç$ºr8?ˆjb­£?ï÷¹`Qú¾?AÂ9:›Ñ?P?\
…)?AÂ9:›Ô4FGL J0429.8+2843?êi5ú$uÀ*óÝüŸù/À9RîؐOnÀ;ÃD°E®@½?Çk9	@` ßs˜~?·‰Hh¤"?¾Ìևá‹K@¢õ:ªú@5PQQ+l?å$Ã9¦¿g¤Ò»VáA¿áhçv¯Š¿ÛuÓáéêj¿äï ×{|x¿è	çàN‰ÑAGNbcu3FGL J0429.8+2843MG2 J042948+2843?íÌìÞo?±ÅÉ¥Ûߋ?±Ÿp™ü€?±ÅÉ¥Ûߋ?珟IƒÚ?ÑJ3:lª<?ÐàÁlùæL?ÑJ3:lª<?íÔðŽm©-?¡Q¾Ý…?±X{Œ'¶?¡Q¾Ý…?ç"+‰)Ø?¯ÂPî²»Ý?Ð÷¨í¬àQ?¯ÂPî²»Ý4FGL J0429.9-3101?Úoú¢ÀEIË>WS¤À:&˜Û-¸ À<r$ëqÔ@!uƁ?ýJ½"så«?½¾¦Š˜Ë?»×xÍFD]?þv‰Ê½f@Ô:®0?ËÍ2xMC«¿Þ¦^c™¿Þí,¾¤ëÝ¿ÓPNâf<¿äò?£%¿ç´v)RáAGNbcu3FGL J0430.1-3103MRSS 421-156568?ïûenb2?@¾;)Ýk?BjFwÓ;'?@¾;)Ýx?ïý7dh£?PQ?\âîê?6Dßĺç½?PQ?\âîã?ïð\ŒK?d¤?û÷üÂ?_FtÛiïD?d¤?û÷ü°?ïØØ;k"?YæÒ¾¢'?s"âJ5õé?YæÒ¾¢4FGL J0430.2-0356¿Üˆ¨^Š—3À@}7\ŸÀ:ÖöV3|À<i²?'ÌÎ@'¥e՜Õ@øá…Áu?ÐRVy‰XÚ?º¹»£К?ä¤Váä-@	ÓÆë|5¿ÐbH_bŽ¿æ(ºžÌßA¿è,PÓ¿î,ma,j¿Ð|T¤Çõø¿ïm í¶QAGNbcuPMN J0431-0406?ïÿáƒC8o>ñJ [4>î|¼Ç'->ñJ [:?ïþõRó2?=oõCÐãö? ªÐÆüì?=oõCÐãç?ïÕr¾™1"?vÔtR%?uF ³g=?vÔtR,?ïþ¢sq[?âUAM~?%ØÏøê-–?âUAN 4FGL J0430.3-2507¿ë\'­ÂÀDFÜ]cˆÀ:0%°"±"À<z"UŒúO@wàÎ'.@0ñ¤óið?¹^€hñ;?œf8n0Š6?ã5Õ¿º•"@¬7ñ³â?ïò+
0À¿ãî!	¿â¹·a*½C¿á;w¥S¿ÝXODù"¿ðAGNbll3FGL J0430.2-2508PMN J0430-2507?ïô¤±½?S'ˆè §?V·ÂÌ'd?S'ˆè §?ïûs«xÚÌ?_R£2_vþ?B1R"Í·?_R£2_vô?ï°ÖJ"Ò0?ƒ§Ïۘzµ?ƒÊm[sú?ƒ§Ïۘz±?ïÍŠ^nß?dñxtªiM?ywºÐȐ"?dñxtªiS4FGL J0430.3+1654¿èÙɃpGÀ5
ȁäq.À9—ˆŠ}œäÀ;ÉLíï\D@dƒÖcÏ]@Ŝ[cÔ?¶#Ú$ÏU?šƒX ¼3ß?ã¤Ô•îê.@ÆîÍӇý?ïý³õerK¿ƒ]$ԚĿæéu¿Ê°¾¿ãڛ!Y¿ãxê݃ÿ)¿ç}d¿È,AGNbcu3FGL J0430.5+1655MG1 J043022+1655?ïôŠl¦u?WŒÙf|,s?Vë&³ÂÑ?WŒÙf|,u?ïý9¸%?Q¦ÍÚÜÝ?62>×oÌ?Q¦ÍÚÜà?ïXÓs?Š€°Î®"?©ù8K#4?Š€°Î®"?ï×@n‹ûœ?a³'Lju8?t_Ⱥ1Î?a³'Lju=4FGL J0431.8+7403¿²íDkhöT@1^‹\¿ôwÀ9ÿ¦å²vàÀ<oLjÀ-'@ýBÝ ?þë`ºU?´åV 9Šª?¥8iRÿ×;?ð£~õ©e@fuÜ{ ?ïÛS]u&¿×^Ÿ"¦¿ãû–yS¨õ¿ØaéÿãzŽ¿Ö•ǶãV¿èÜ)áû³AGNbll3FGL J0431.6+7403GB6 J0431+7403?ïþ[Ðܱè?"h;LX%?*Bò4á};?"h;LXL?ïüþF6Dî?S›Ú<ˆh)?8
ÎMؐŠ?S›Ú<ˆh,?ïõ•¢^_8?]ꓣõ3?TÔ»CAò?]ꓣõ0?ï÷Œ»S?ý?;Š;k"³?Pæ‰Y€	ª?;Š;k"¢4FGL J0432.0+1732¿í5kȪ5åÀ4U.ÓÀ:ÆYåN£ÒÀ<pz¼^À@îQ†…j¹@Á]¥Í"ƒ?Ô'øR¸?Ûß©~+V@µ;ÑgfA@"pµßö? S~œÅ¿å(Уñâ0¿ÜÚsÿV6î¿çLê"]ðv¿ï»batE¿ë¥­Aí
AGNbcuTXS 0429+174?íU7V' ?¹2À?µVEKnÿé?¹2À?îhû×uˆ?ÁN°KÜ|?©pBŽh§m?ÁN°KÜ|?éù=lÈã?²k¯Øá?È
LÜs»?²k¯Øâ?íÌt;Ô¾É?˜ïíQ?±œ^!Z	Â?˜ïíQ4FGL J0433.0+0522¿Ñhžsf7À;j¡è´lÀ8ôxmÏç4À;œ=þhP@4@§ºï€@st¼j~ú?²‰`
0ë?Ðý ¿¨¡õ@×õûn@…¤Q¦ù¿×›X¶z{¿ãìÓu]¿éÏ^âäfG¿ìª$Ìh"ÿ¿ð?ëí×^v-AGNRDG3C 120?ïçì0…¼[?tW"³0-5?hÏzC¤?tW"³0-1?ï÷ÌÖX§â?aiE© ?PfSN°>w?aiE© ¡?ìƒPg"I?¨ÿÆg¹Mí?»å|ÃÝ·,?¨ÿÆg¹Mì?ïõy°¹?KáDÆP÷?UÉçžŽ?KáDÆPã4FGL J0433.1+3227¿È"°é®>ôÀ$åi+<ĬÀ:7®_ú;›À<(<üàÏ@!A¯à+#?ýhò	1?ÂP?§¿!?¥Ùr€-À`?ãn;¢BŠ"@ˆ™úg±?ïìŸ/ۏ޿ê.8!¯}1¿á¥îaG¿؟Úép¿Ö
µ%;Mß¿ç› Yý!AGNbll3FGL J0433.1+3228NVSS J043307+322840?ïý¶
`©5?,'þÅöŒ?2O¬ú¶d%?,'þÅöV?ïþAç+Væ?Hw7¥zr–?+áJ'šã?Hw7¥zr'?ïí»=‰WÀ?p¨Ú½?ú3?bDÂv¨?h?p¨Ú½?ú5?ïàn€ƒ#V?ZQ^H¼hÐ?o'|Ü©ª?ZQ^H¼hÌ4FGL J0433.5-1039?è÷`\-6ÀA²÷üü?À;vºq€vÀ<˜Fíû¾@éEÔJ›@'µÿ_Ç?ÈÒ»y=X¦?®ßM>2{ä?àˆµENJn?ü\±+†–ˆ?ë.-9ôîT?ç­½"4Þ.¿ã&ä¦f&¿ãñV^ÜY]¿ïòbRÛo'?ïGÿ¨Â+‰AGNbcu1RXS J043333.5-104220?ïˈ7(+^?y¶zæMH£?z;äkêPÜ?y¶zæMH¥?ï¤Üm©p?•܏æ•?†Èà$•¤	?•܏æ–?ï	L>ÄÜ?'a«Ø;Hû?žßvx'd¢?'a«Ø;H÷?ï4Ç=nÛ;?÷BúÀÆ?™gR$˜ž?÷BúÀÆ4FGL J0433.6-6030?èÜ
¬Ê\ÀD5\ÙëÀ9Cº­˜#À<!.b@ݝ^ä'@¨— B•§?¨îL¤Ht8?À³l©v†@:x¯>F@¨Úã:øO¿Ëç*Üw¯¿Üp5½Q.Ç¿æM±>&p¿çÒÌ ×üV¿ê"—8w¿ïýÚV"K"AGNfsrq3FGL J0433.7-6028PKS 0432-606?ïù¨DÅ6?C
=C³¡?I_êìë)æ?C
=C³'?ïøC&†ß°?r/+?NóeäCç?r/+Œ?ï_'Í°æ?'2ÓŽ0ï?"
Æ^‰ãA?'2ÓŽ0î?ïøÙÏË5ê?:å.¥«ýo?L˜ÀÓ(TÔ?:å.¥«ýˆ4FGL J0433.6+2905?äzÓYtwÀ)3¤r:¯ÿÀ8\iñŽMÀ;9îיå@1ºv^;?ÿ²lHþv"?¨	Ê?eò?¶ÜÝæûw/@e^è¬@»G»ÖZj?ƞÅ''êN¿ÛnÂ@öö¿àobùÊ[Ù¿ßÄ-ÁÚ+¿ä!¸âÓõ¿ãH݉³r‰AGNbll3FGL J0433.6+2905MG2 J043337+2905?ïý¸%ÊtŽ?(tAøÆ?2>Ѭ[‰ž?(tAø$?ïø±ÅU:k?_õP/Þ²?M8ê«XG?_õP/Þ°?ï½1^@3?"㞎Ӂ?€³¨oû³}?"㞎Ӂ?ïñƒ=|"?Kßp_åý?]Æù…ÛQ?Kßp_æ4FGL J0433.7-5725¿ïӟJ)FZÀDvŽÞT´À:Š:ÏߦÄÀ<š©glö£@_]³d?úBfýe
?Àé(M&#€?ÐC†g­Ó@àÇÀôQv@Sn9œ?ïèC ¾¦ï¿Çq¾ß#fŒ¿Án+ALP'¿Üɘ$y‡¿âw3"«C¿ës,è–VïAGNbcu3FGL J0434.0-5726SUMSS J043344-572613?î˜PAX¨?¨ÿ¶Û[E
?¨zûêuˆ?¨ÿ¶Û[E
?ïÕw'éùÉ?'Ám?i5Ä?uD7?'Ám?i5Ä?è	+ŽPv?´Z¬
»Þÿ?ÏÛS­Æ¾)?´Z¬
»Þÿ?ïÿl{͋?…9՟¨r'?œàp†N³?…9՟¨r€4FGL J0434.1-2014¿Þy0ºPÀCzÞô¾À:>))ÄõhÀ<"VE†òÎ@&.iIð@4FY€¥?¾£eூº?ÆJL)y@f¨Þ°û@	éaþw¿ª¿ë¦œÒþ¿¼ÍfC½¿áLýpÇ¿éòB<»r1¿Ç^,»C¿ïÿùJYQAGNbll3FGL J0434.0-2010TXS 0431-203?ï÷^ƒö>:?Vµ@œ¢Ñä?QBøƒ‹þ?Vµ@œ¢ÑÞ?ïýèÅn=?Jó‡‹ñj$?0¿!ԎŠ?Jó‡‹ñj?îÝàäܓK?–	ٓ–õ"?¢!ñ²6ËA?–	ٓ–õƒ?ïôTOwŽ"?L;s*2óÂ?WWaâ×H?L;s*2óÕ4FGL J0434.4-2342¿ãð*y.tùÀCùáuÑ=À:{k*ñERÀ<ˆ]
ô@t/"î;@¼'Æ#?Â8MyZ‰ä?¸IàsȤŸ?óIxÔýó¶?ÿþGn(¨?Õ%‰&"Ï¿ã‡"ØaV¿æ·k;¸<ó¿ã6_mMá4¿æ:®â¬/¿ðAGNbll3FGL J0434.4-2341PMN J0434-2342?ïïÀ®œ01?X–Vڋ¸?`?QcÏΎ?X–Vڋ±?ïÐYüA¦X?/ÏÉy¡[?wÓß,Ô!?/ÏÉy¡\?ï«$bwI÷?)Âðþcm?…6çb-'J?)Âðþci?ï3§ØMó'?'˜³p'?™‹öA›&?'˜³p'4FGL J0434.7+0922? ‰KÚÌÀ8ñ|å-íÀ9—b=⹞À<ˆv[¦ð@ RGS?þ9¬CÀI1?¶¤u7d›?­-rð³*?ös?wåë@0»O÷º?îÄâÞ0¿ä/P…S'x¿Ø,¹¼¤¶ƒ¿Þ0{rçÿ¿Þ\ÐERD›¿áÜP=Z(•AGNbll3FGL J0434.6+0921TXS 0431+092?ïþž^W}?0TkJÐ8?&ˆ.˜?0TkJп?ïþêC6Š?A%ÿ/£mð?!^̗m?A%ÿ/£mÌ?ïö%{ù"Ç?c8Æ(£?SµÖp­?c8Æ(¢ü?ïö}RÏü8?@D*¸¶?SZ`ŽK?@D*¸¸4FGL J0435.4-2623?êßdzþùÀD6ä:§›»À;OÞÉN"À<³fZOØ@¼{päš@!G®zá?Ê-ªɏV¿'³Í;Kta?Åû€ÿÄÆÄ@xsŒ>½*?ë¸[#*?îì1¡¸¡ó¿àµpà<ì¿æû½¥h¿Û¯ùWoRž¿åQ‹
ÜAGNbcu1RXS J043518.7-262120?ïÔESØ?uíøå€õ?uø{ÝV?uíøå€õ?ïøºBmfò?j"ܻÀj?MöJd;?j"ܻÀl?ïP3ê?æ?ëÈA»ô^?•ù'¸<I?ëÈA»ô]?ïãf?û?]ü—亩?lý™À~B?]ü—产4FGL J0436.2-0038¿Î)Ö(DÇÀ>›Ã?…QÀ;«ÆÂǐÀ<¤Zk†`Ø@¯}óJå×?þ"þ)f*×?ÒZžý0ÂÁ?Üÿf<Ÿîr@êf}ãZ®@'§Dýàì?É»…õLô?܉uʇx/?Ë| 7 ¿ä',ëp¿æÌÁd8å¿ïöBmbÚAGNbcuNVSS J043614-003637?ïÞñËÞL?n£ã–Ô?p‡ÙûÅ?n£ã–Ô?ïö='6!7?kh(šøZ?S"Ý"½?kh(šø_?4a¨Ã?›ÜÙ¼ê?§´ì¹åsÀ?›ÜÙ¼ë?ïÚC5 E?†'F‡tG?Ÿd·™K÷?†'F‡tG4FGL J0436.7-7148?¼"é𩑰ÀAûÇ£˜ À:ÇĹ­À<‰‡¿}@ð¥¦Ã"Õ@úR¹á7¾?Ä1?¾
†?¡J=CŠø?ÜYÀ@Lv@¬ó±³?ïö!úü‹¿ãë½RÜF¿åòCŸ'Æ¿Û ë™á¿é\,9
ä¿ähF&*AGNbcuPKS 0437-719?ïÝh?Â!Õ?iÃB:ùè-?qKàï4?iÃB:ùè+?ïù9jòBÓ?[Ò«–Dz?KT6ô²ð?[Ò«–Dt?ﳂC|3»?'{e–»?ƒo ó?'{e–»Œ?ïÎ&ç@ë?bk»©Çè?xìŒvߊË?bk»©Çì4FGL J0436.8-5223¿ì;_ÈóÀDºëp&ÉÀ;x¶ËÈÀ<¤FvÜÖ@+}‹Q@Þ0å{|?Á҅ÉX#-¿³­FàH?ðÆB‰èK®@
¬Tš.‡¿åCªåx,¿ë‡—Ù¥ù#¿å>™=~:ÿãx^Kò¿ïy4i"P¿ïúâm©QAGNbcuAT20G J043652-521639?ïÿ3ŽA"?!#aZõõ?Ž=÷ÍvË?!#aZõá?ïýuòé"æ?O'¤x
?4Ph³`Ӝ?O'¤wý?ïé{—«€Ó?j)±³õën?f"hT,R?j)±³õë‰?ïûåð/C&?3Ö}»‰ø	?@h?Bói{?3Ö}»‰÷Ú4FGL J0437.2-5846¿¸|8`.öÀDØ@žUÁÀ;:†—DÀ<—7£|g@ûy¹h@`V#ùŒ?ÇÝÌ#""z¿š¡éŸ@x?Ñõ몦?ý›Eìu?áŒwr¿ét ά Ý¿ìx¨B~՞¿È§ùÈ-¿éoîo´Ã¿ïü–ž½oãAGNbcuPKS 0435-587?ïðº<Dî?]ÃÀœ‰²?^‹‡ãv'À?]ÃÀœ‰²
?ï±}ªïÜ?;0*îk?ƒ •DúÖ?;0*îk?½…ñ"?†­.¨ Zø?ßPžƒŸ>?†­.¨ Z÷?ïȉxa^?kÄ®ÄáV¶?{»CÏpÑF?kÄ®ÄáV¶4FGL J0437.4-6155¿äþ@Ćx´ÀC§´ÃÁ‹PÀ:ÄC͵*À<¿	A=@ŠŠ}òÊ@>aÝj©Â?ĕpªä?¸± Hõ½1?òÊɽMÓÈ?ý÷børÿîWZ$8Äm?ȵ˜¾'m'¿âJ¹—e⳿ä5V#"Cø¿à| 9›Ø¿ïþb¦¾EKAGNbcuPMN J0437-6157?ïñ~;4Ô?W hc³R?]‰ã–U£?W hc³K?ïâöJ*5"?‹ðüõÃ:?m	µÕÊܼ?‹ðüõÃ;?ï—"ÉêãÛ?ƒ¨ª.q?Š7M…G	u?ƒ¨ª.v?ïoˆàب?€@f…Ã?'ãýdë?€@f…Ã4FGL J0438.4-1254¿èH'™Zò;ÀA£.3ðÀ:‡;ibš)À<^÷ÇLZL@»Ç<êìó@.O[‡æ?ÃÕgûè?¦ÏÆÁã?ävÓ xñX@p¾µ²ÔÔ?Éص¹4êm¿ä¨¿¨!¿èqÐý³õe¿Üv<eç¿ìÊkÞöE¿ïÿûÎBÓAGNfsrq3FGL J0438.3-1258PKS 0436-129?ïþ&ۀ*?%¬:?·?.'GýS—?%¬:?Ö?ïÿ{àǙ?>#i¹¹3±?ðƒçæ|?>#i¹¹3³?ïìñ¥S¶Ÿ?m¥d6ÓG;?cZ¬I`­?m¥d6ÓG)?ïüR÷ëc?/kJâŽR–??½h@¤æH?/kJâŽRÙ4FGL J0438.7-3441¿â€úŸ£
_ÀD¦^5?|îÀ;"xt…äÀ<ãJ?¿2°@!(dC '?ûë÷j/HÃ?̈éH-–;?ºPÓZ?ð¦<åd@›‹9¬³¿ïù_‰X?ïúµ´)h?Ù®åRп½ÕçRµ­¿ïÿÐÐgŒ?ïÿ	àÔk¨AGNbcuSUMSS J043612-342230?ïÿW2õÔ°?©àÆ¹?¡Eiúµ?©àÆÍ?ïüäÍÚ»?UçÙk	ˆ?8ßÁ'*$¤?UçÙk	ˆ?ï¹ÂY?ŒȖñœ?Õi"?ŒȖñœž?ïð"†ËjÌ?WÀ~ý"ú÷?^Øòi*j¡?WÀ~ý"úõ4FGL J0438.9-4521?ì.âWâƒÀDâ$ p¹À9N¾7ޓŸÀ<Nªaâs@¨ªÙ‡ñ@c¤G?¬™šròç?¯­Hß(*R?ÿ —Œ™@/&3E|·?ïþŽäÒ}¿ãþdßӏµ¿å}U¡E¿ç0§g¸uþ¿ç­ý~ÆY–¿Ù³œÅH'AGNbll3FGL J0438.8-4519PKS 0437-454?ïþ'÷°?#4l¼kA??'ސ"ÿÎe?#4l¼kAq?ï÷ÎC@?pëV§¯Nn?QÚcyÏq?pëV§¯Np?ïÚAöЬ?n''ˆ—ìõ?rûß—©¬?n''ˆ—ìé?ï½Ñ"Y[7?n̋ÌPTØ?€‹·i©2S?n̋ÌPTÝ4FGL J0439.2+2151?وæ0ÝÄýÀ0KL<µÀ:V3sÊÒøÀ;íK¿3@çښ?ܺ@¬Ì¤ˆàå?ÑÈ3'˜?à¥e¶™…@ql¤nò@X¶ÄLˋ?ïþ8µS3"¿ã¹]¯2³¿á6,!qé¿éò3¿ïúÝ¡†M¿ïÿR@>´qAGNbcuIERS B0435+217?ﻧ%[€r?ˆ\~	°K?6©ã|?ˆ\~	°K?é¶X"Ó¼û?ɶ2nÁ?É&¬±?ɶ2nÁ?èã*…@Ö?°èìQ"?ÏÀsUêüª?°èìQ"?æZÆJBÂ5?°áWàWÇ(?ÓJskz{—?°áWàWÇ(4FGL J0439.4-3202?éH@A'0ÀD_鞔«À:}WƒÀ<†"¢¹ÓÌ@ßeSÁÉ?þò?¸|³°?¼ÂSw rç?6¨ÈO~?Æh®ª¢ÖY@±÷ò"ò¿å@XëS '¿ÖByaÀºE¿ãÜ'"€{¿Ý k…˱¿ÎÌû›Â=ӿ䔦 h?ÚAGNbcu3FGL J0439.6-31591RXS J043931.4-320045?ïýÎèÚ?2'ȳòy?7Áˆ¹ã4Ÿ?2'ȳò{?ïþ¦vðÈ?F{ï=:Ü?%˜ó',?F{ï=:â?ïóZ‹—æ?d'vúʽÀ?XÅJèÐ67?d'vúʽ¦?ïýaÁ_o?(ÎïÓ<ä?7Lñõ~€?(ÎïÓ<Z4FGL J0439.8-1859¿ï'Ø
KthÀB¢\þޗÐÀ:
lâ˜À<L›ó-u@؉À]¨¨?ü*î «†?»"(k"Œ?¾Íç©òØ$@}¢™ó\@?'˜rÓ?ìÓ}c.¿¨Ç(H¦¿àÿV"tn¿Óeî[è´	¿ãó·‡Á*¿ßqoC"ºAGNbll3FGL J0439.9-18591SXPS J043949.5-190102?ïéCæ,?iéÞXÑ#œ?f¼êë՗?iéÞXÑ#?ïõ,þtO,?i³-J\…«?U¦a¨'?i³-J\…¨?ïÆR45y®?'{ç#O?|ÖååC)p?'{ç#O?ïZ'Ñÿö?||/W¥iÈ?"­¥ß€R?||/W¥iÌ4FGL J0440.2-2458¿Úr€0vÁÀC‡+À:ªá»qZ¶À<q¯x(/Ê@!²§'h˜?÷<Æúû´A?Æ-—<òú‰?ÆêÚÿÀj@_l&™Ç½@ßDd¢¿ïý;)¡¹ú?ïý¯žÐ?݃¾š?¿ö+ëÁ.´¿àÏìÝ
Œ°¿Ê¢Âiq‰AGNbll3FGL J0440.3-2500RBS 0570?ïó*F'à?RA
â«?YÕ«s°@?RA
âº?ï÷=c'?l'¸H¦x?Q…Ó9ﲃ?l'¸H¦{?ï ñ1µL?…4Â_€&?‡Ã³'ºí.?…4Â_€%?ï•0—¢?zû¾`ÄP?Š³Ü{Ä?zû¾`ÄQ4FGL J0440.3-4333¿ï/"ÜÜÀDÆÙßÚƋÀ9¤*ߧšäÀ;åíùm@¦'€x`d@³õ€J=;?¹»æàõ"×?Úù\ã/å¡@C!°9ï@Â=Л
¿åEÄe>Š¿ÖNØ²´¿è™'6É?¿íM%'pˆ(¿ïÿ‰b"ʨ¿ç€VÂYQAGNfsrqPKS 0438-43?ïAÚ̞?£`)°†ýÉ?œ÷Ħl>€?£`)°†ýÈ?ïödÆ5¨?m>á"¯?S÷6s"°ï?m>á"¬?耦ª#ûi?²‹Êù3Y¦?ÍýeWp[?²‹Êù3Y¦?ïö['?NKÿ¡JFU?SIËãÎÜ*?NKÿ¡JFI4FGL J0440.4+1440?àÞv,:"ÉÀ4~=jΫÀ9ߨ‡s&À;³\ÜJ@;2ú(P@ÿV"tn?ÈÖMªñ?Æø´FÄ	°@;{Q^—?ýig…d?ï^"ð•(ò¿ä´ÔÞi,i¿Þù‰ƒÌÓ®¿å†D
K¿êGq®™¿ïþaAGNbcu3FGL J0440.3+1444TXS 0437+145?ãà+·Û"?ËbÓ«IJ×?Ø?¨IÎö?ËbÓ«IJ×?ì7›ÈC?Ä?DÞK&?¾C'I½ã"?Ä?DÞK&?ç@Ó[ç?·6v¿	‹?Ðå~YIÌ0?·6v¿	‹?å,Ý–t?°EcUÁZÂ?Õ§ÂEÀÓ?°EcUÁZÂ4FGL J0440.8+2749¿ï7ì.«gÌÀ(n~¥øL­À9x
†Ñ?ùÀ;éò‰õ·¨@ $~Pg÷`?ÿU0cu^?¸ÞÎWˆ?¸ç÷±¡@Ⱥáè½Ä@6ù8¶¿æ£ùdo¿àTl~Xu¿ã…‡"ݘ¿ÚÀWVP¿Ù²¾c}}Ú¿ëÃßóðþAGNbll3FGL J0440.8+2751B2 0437+27B?ïæÅÃå:?e¡G]2Ñ?i:<rż?e¡G]2É?ïB?«…D?µ	ýÓ¯d?—¸
W=?µ	ýÓ¯c?ïB²ZÙ?'¸`|÷")?—©¿¼Ô¤ö?'¸`|÷"+?íì!Εý?™âàL¬Aç?°žñãP?™âàL¬Aæ4FGL J0441.3-2617?îÚôœ'rpÀCÅ'U°6À;ù>U¦$ÂÀ<ý/iz@"_Ë1í
	?ø…ÇŠm¬¬?×ýÍáéO?Ân³|n»u?êG-ñªÒ§@|±¬_ð?ïÅF%~>Ê¿ïç7a–
?èìcÔ¿àùþ"ï6¿˜¨[ÜÓ2Ë¿Ò`UÀ¦Î¶AGNbcu1RXS J044120.5-261659?ïþÊ}ûՕ?#¯%#ØH?#X B¦Ñy?#¯%#×Ï?ïþj¼'ì‹?Ioâ£ñ5?)T6á7_Æ?Ioâ£ñ5ª?ïäˆÂ3y?r÷Lò¬Í?kw=ÌîˆÚ?r÷Lò¬Ìþ?ïû¥×i?@Lm$´xÛ?C•iˆ¢Zµ?@Lm$´xß4FGL J0441.5+1505?åkj°¥xnÀ4	ü›ÇqÀ:RžŸ'×ÞÀ;ð³£¼@!ÔE¼ø™@<êòQÁ"?Á™#RŸÊ?vX\ÇÝù?¸]†Ð&?ýòº‡¥Ñ5?î]'"ƒ¹¿ÚF\»lӿ七Ÿ\Q:¿ã—d53¾s¿×ü}"€U%¿àìm|]]AGNbll1RXS J044127.8+150455?ïá
éÖ?k"öòmÀ¾?n€òý)4?k"öòmÀ´?ïóTw4Ž?pöksh¢?YWÙ–âÕ?pöksh¢?ï£}Oԛ¬?"ðõvÕ[?‡ ¬
Ù?"ðõvÕ]?ïr	?yu?~<‡ [\=?'¾ÝØђ?~<‡ [\=4FGL J0442.6-0017¿èu#|ºÔÀ<v\=îxÀ7æ#ú±À;¦$p!Ñ@4{;4´h@ßýç!é?•@†Êñ?±¯=oÍ@ÃÀ;ÄÒ-@¢…pµȿÓc?ò©€¿ãYø™Ú¿æ\Ëè¡>ª¿æ••"z›¨¿ê¡Ù¿#–Þ¿ïþš¥2TAGNfsrq3FGL J0442.6-0017PKS 0440-00?ïýöö3v?&ÚÄãˆÆ?0HNdO@¶?&ÚÄã‰?ïúGv·?\§ðg4µ?Fâ%ù#ã?\§ðg4¿?ïÎ6Zuuã?xJXi¡?xäÒÅE§?xJXi¡?ïÿ'tû{ü?­XîN ?bÁ!ÕÚ?­XîMŠ4FGL J0442.7+6142¿éë¢=ƒ@$^°ËæÀ:2"ѼsÀ<:ÏߦÄ%@ ö}¼ÄA?ÿÀ©"£˜÷?¸F x[Š¿u-¤Òîá?¾¢8FîQ?ú"êpvµ"?âÈ9À.¿®¾NÀézê¿çf>ù:!¿ØïõÆÁ¿Ý"F¡$'}¿Ö¨À(#¶AGNbllGB6 J0442+6140?ïÕ¿†Ù?qôX&À?u <û"qÀ?qôX&Â?ï©Á¢À‹a?¬é‰(>%?…—OÝ( ?¬é‰(>&?ïѾ¿¹³«?xц{òØ4?w  #&*?xц{òØ5?î»ÞôXä?Œ`Þáé(?¤B¾:qÀ?Œ`Þáé'4FGL J0443.3-6652¿ÆŒ›m<ÀÀBš-û¹À:@èþ[»À<t>ÿðÈ@û>¥,J@'Œ¢:R?½PÓs?¼f7íW1?ü°qgKh´@
ëc€­åV?ïúŸmîðä¿æ¸à0×¹¿äƒ`½Z¿æ=ø=éŁ¿èè®	"&¹¿ïÿÿ&¦³AGNbcuPMN J0443-6651?ïü˜
[?6aiwÎû?;?Ÿ­'!K?6aiwÏ2?ïþ6b-t?D© H—`ú?,™Ý.˜Ñl?D© H—a?ïÏq…膽?te¦'‡W‹?xG=¼¡2?te¦'‡Wˆ?ïï"|ìâ¤?K~ãý.BS?`݃[Ð?K~ãý.B`4FGL J0443.4-4152?ÙÉjEàc%ÀD{BB…À:ôG1ùAÀ<±æõlÿ@ €ö|²Ã?û…‹Z;µ¹?Ènþ"n\?¿"xuœ9?öÑPüDŠ@'°f·š?â=Œ²­è?Üæ´yý¿â©ö©L¿ÀÉljÁà5¿ã»aÕÝ퇿ߪÛá<ÆZAGNbll1RXS J044328.4-415151?ïõá.åQL?Rz>·°'$?T=¢5]d¡?Rz>·°'#?ïù…ŽB?bxK$ˆÀ?Kýë…Æó"?bxK$ˆ¿?ïêÐÄ9¶?fÜ+-Aåç?e/;ÆIý]?fÜ+-Aåè?ï²4LJ{?kc"/L»š?ƒrûŽ!B?kc"/L»›4FGL J0444.5+0719¿Ðù·ÇQ¬ˆÀ7ô§Å¬GÀ:W«(7V®À<"O¶
é@¼R˜©.¸@yŸâÚU?ÂVy^e»ò¿›àûF̆ñ?×>;"»f@	úõÕÓ¿¿þëWýB¿çÒ(¡‰Òý¿ëeHŸ5Û¿ÕñŠ;­«¿ïÿñAÌ(7?ïý ¿¨¡õAGNbcuPMN J0444+0717?ïÿ-è? ™9R+N{?NbýM? ™9R+N§?ïýèïÚ?QtÉáÇð ?0¸‡y/ͦ?QtÉáÇð¢?ïߍ˜›`ò?puüْcþ?p93²O†"?puüْd?ïü¤7Q,ì?1M[ª~6?:ÞEv˜ªæ?1M[ª~*4FGL J0444.6+3425¿¸ÆO¿|¿ÀmtO]5eÀ9Ÿ¤¦=À;¸Ï-Ðã@à²;Qæ@™ÐcZBl?¼5ŽäÒ?­ê4"ö?óÙ&­ó"@M£ÔfÊ¿»j^˜'±Ä¿Ò£®Zñ¾¿å^ü_ag¿Ü^î7€ŸÎ¿è,	æ~O¿ä»ÁŒ§ÄAGNbcu3FGL J0444.5+3425B2 0441+34?ïé,žø©¿?fÖÞã*?fÓaV@œ?fÖÞã$?ïü´ i3?^UJÏ·é?:^ü¶c—?^UJÏ·Ý??Ã?Š™	Ù"?ˆ\ú¼p1?Š™	Ù?ïÀ:ɈŒ?iJεGÞ
?â›<¹'?iJεGÞ4FGL J0445.1-6012?ï"©-S²ÀClX£/D'À:£ó}:¾BÀ<®þs8@ìVò8Â?ÿFŽ¾?Âæ¹G‰×Z?¸`ÏΉæH?õ>.‰€Fâ@	lY夊?ï›h zÉË¿êÑùÝQ)h¿ÙJM@¥Œ—¿ß£ü>Ty¿àŠÕ±wÝ¿çÕøÅyAGNfsrq3FGL J0444.6-6012PMN J0444-6014?ïÿ¬"Ų?
³©ÿ72?؛"RÞ?
³©ÿ7½?ïþ ¬ÙîÎ?M^S3EÔ?-õ2a?M^S3EÈ?ï÷t
^Ä?gGíš-‰a?QåBy"?gGíš-‰\?ïùÿ#md?6.­Wøúw?HïrJtœ?6.­Wøúj4FGL J0447.2-2539?ê4zYaÀBÖ5"_õÀ:ØøúRAÀ<¨!S6Þ¹@Øée´»@>ª¢ÖY>?Àh‰@ÛèI¿©ÒçÃô*?êÇ5žd?õ'¡Æ
ëÑ¿àôÈý¿Î(•µßJ~¿æהܛvé¿Þ)–|XÁ¿ÞµñäíU¿ÔÖ[[	fAGNbcu3FGL J0447.1-25402MASS J04472149-2539302?ïô®¸UEƒ?P«1Í×zI?V¢Utùª?P«1Í×zE?︮Rn=?–‡	vU_?Ôëdp'?–‡	vU^?ïØR½²ñ×?w"WÛÖï!?sÖ¡&‡ˆ?w"WÛÖï$?ïmͽa?~`–«øH?'FH]\SÕ?~`–«øH4FGL J0447.4-2747¿Üˆ¥Ý
yÀCbäѦÀ<SxM¸À="—jpÐ@ßÀ‹@ÓM"îê?Ø«¿Á¡u†?ïô%Á°Žÿ@Ð=0ã@
òi™ÌšM?î}I׺f™¿ítw Gô
?Û
Ú¤{Ë¿ëžñݨg=¿ïíØë¿[¿ï PØ_¨AGNbcuMRC 0445-278?ïåØҕT?}në2R'?j'-j«þ}?}në2R'?îѶŠÁ"?¼ŠªÍ¼L?¢ä—Sï­ï?¼ŠªÍ¼L?êéÔ3aCZ?®K¦së%?ÄX¯2zò›?®K¦së'?놊n¸¯´?²€P1ƒ?ÁåÖEA/?²€P1ƒ4FGL J0448.6-1632?ÄÅu—7ÍÀA8:}ªOÊÀ9mÆÚD""À<OËn@/=ƒC@ò?ýq½¥è\?±]!™,â?­r¡L%@!
 ë2@aTåµ{ø?ïØRÂD³Ž¿Ê¥ªžú'¿à+ÄÿÎ׿¿Û6QØ7¿Új©Ø«þ¿à­#^ÔÌ¡AGNbll3FGL J0448.6-1632RBS 0589?ïüxsâÓ?5™"©µ(?<<`ï¡uÏ?5™"©µ)?ïûã¼Þ͜?Wöwn*¶O?@q"É–?Wöwn*¶U?ï켬La?ibÜ)¿¢?cCýS³žr?ibÜ)¿ ?ïÉ=÷g?bÛ ܗ?{awÌ|ã?bÛ ܗ4FGL J0449.1+1121?ÞâÝNæ'À4¼«Oœ À8-e•†¢À;'·îvï@¶Ä¼2ã@ewS?¡âއ	t?ÁÇ­¾"¥¿@©qÁ
{ê@À×õŸÔǿјº¡|¿ámm "Êþ¿çga8)<¿ç¿]¾L+}¿ì§%pÔ)¿ðAGNfsrq3FGL J0449.0+1121PKS 0446+11?ïìȄ֐?ˆÙˆl¯v¿?cû7{)qy?ˆÙˆl¯vÀ?ïÑéÒ^¥?›Ð
<>R?wy–Эœ?›Ð
<>P?ïiñð·òÝ?×MðF'N?'ÁÁé¤]?×MðF'J?ïG5¬	?'ʖEd=?—üùJ~à?'ʖEd<4FGL J0449.2+6329?—ýc5¼@'Ía€M˜9À9']Šõ'À;¬Ê‹¨?@ԂTƒí@íhžO?ªÐNâf<?·AªoT̋@Cf½Ë¨@C4ò% ÷¿Ú%a#""¿Ó**@Ejm¿á³hãh­¿ä¡÷ÁÃu¿åÎÀWs"\¿æž£Ä•ÇAGNfsrqS4 0444+63?ïön¶®‡Þ?N›ÌNE	?S"'¢ðE"?N›ÌNE?ïõ¶bÏ?u:èíBx?T"Ñé:dã?u:èíBx?ïW:xì°?)ÂIñ?•¼Pâiì?)ÂIñ?ïÿkbÁ?/¨*š2?"§Ý'.?/¨*š4FGL J0449.4-4350¿êœáÜ×eÀCõâŽÕñÀ6ä˒:*À:À>ð֗Q@vµú£IÇ?ûþÛ<Òf?'¯­|r?¯­DË@Ö"Ì«?@Lêt'š?ʜ­	ãل¿Ó¥"EO@¿ÜA¤ÕÍ¿×ÅP׈èq¿á*½]Äu¿ÚôZƒGsAGNbll3FGL J0449.4-4350PKS 0447-439?ïó䲦և?[0þ(kÐ9?X6š²Ròæ?[0þ(kÐ5?ï颞Ÿk?z²ÞÅê?f]a`ä•P?z²ÞÅê?ïˆY̦?'dd"ºc?ÿé¾LÖÄ?'dd"ºc?ïæ)³ÌÁ?[O¤›ÿ¶È?iàÖL3>?[O¤›ÿ¶Ï4FGL J0449.6-8100?½ôç‹FBÀ?cà·õ¥À;À´%tÀ<ží$[)@ êÿ	àÔl@¦@×`¥?Ãþa"Õ<]¿½n¤ÁÁ?ù›ÞM'Ðÿ@*¸¡Çx?ïÿ¡ÁnT¿ïˆ_µr=4?Òed®¿ïõYÀÌä¿îO²
¤Ÿ?ïüV'TàAGNfsrqPKS 0454-81?ïýoò´?G¦ŒÎ¡žË?7ä‡jaD?G¦ŒÎ¡žÂ?ïß<źmw?'"‹7Рš?pa"ÉDÁ?'"‹7И?ï¼>=%°?"+(9²ù
?ˆx8[Iû?"+(9²ù
?שּׂըðz?€BÕöÄéã?"ÔŠ•Ãá|?€BÕöÄéå4FGL J0449.6+3027¿ßîýxÔ¾¬À"GýœÀ:4žÝ¦8äÀ;¸sQ0t<@	=-.@¬œ[ùŒ?Í/5wÜ?É9(Ö
b?þË|j´ª@å¨îÌ&	?ïßG"Ô@_¿å%èâ­â¿ë@óæ¿âW'X\¸h¿ïéÄ¿¸T¿æ$AÓ´óAGNbcuMG2 J044950+3026?îerÇK?­hLÆ/Š?©¨Ó¯ëK?­hLÆ/Š?ï4¢áZ¤?¯…®$Ñõˆ?ž™k£Ô«"?¯…®$Ñõˆ?éF(dôúp?·ŒÁGŠ')?Êç^l,B?·ŒÁGŠ'*?îï¢^MÍ?"=tE¤^?®ÑÚ#'?"=tE¤_4FGL J0450.3-4419¿ÓüL¼F×ÀCáþ!ÙnœÀ9z:э%îÀ;¶íª'æ!@\‡à‰˜@I©|e¬,?¶9Ô1;·?¸}BöÊ¢%?ûÕv¿yþ@æ}"¨¿×XÝ|Gy;¿äÓI¨Pí¿êŸ¾vÈ´9¿é–ß?–¿ìs§A¢â™¿îW…BI¦'AGNbcuPMN J0450-4418?ïüüлxË?8ƋÜêå¦?8z$9ŸÕ?8ƋÜêå­?ïýöË»JÙ?HÔÈåq:?0I¢%©8F?HÔÈåq??ï|Üßâ8Q?ŠçË_…ð?dd¸õò?ŠçË_…ï?ïøÛz®0î?>¹QYê?L'G<GÓ?>¹QY°4FGL J0450.4+7230?ì.qKó@1x¢Ûa»À;µ'm,À<¦µ™ª@ê«5ÎC@Å+M‹¤?ÆölXmÕF?­‹RY?ãIþ†ƒ<`@¿̀ø?ï¢S².»Õ?ïä>ÙY£
¿ãÕµ¿'¿å&ÜÛ±¿í¬=Æþ?ԁHŸ¬RAGNbcu3FGL J0451.6+7231NVSS J045109+723014?ïémâ{Ž_?boÒ?f'"q¡Š?boÒ?ïó½DŒ]¤?rÜa#‡?X…vçD¶˜?rÜa#ˆ?ï?ðsÜH?'ÙŽ9}^Â?˜ñŒDv÷?'ÙŽ9}^Á?ïÏF߇¼?lK‰¿†®$?x\û<"l?lK‰¿†®&4FGL J0450.7-4938?Ô2z¥æÀCÉúëÄÙÀ;Pûð¦Æ©À<ßþŽæ¸0@¬áUoô@>µÛ¿ê?ųZµÙ[¿–©@€£©h?ÐëÙ!ÄËÌ@Y¶o"5Ò?ï|š…Qãø¿ç8~–ÞÔ6¿àžvþdŽ¿äZ^»w9ó¿éÀ:SÜ?¢{•w öAGNbcuAT20G J045102-493626?ïʲ~£-?v‡ªçYÿ
?z¦Àó®hñ?v‡ªçYÿ?ïøž10;K?ht âG1?M‡;?ӏ?ht âG5?€½?‡µ°ÃŽä¸?_оø?‡µ°ÃŽä¶?ïðzšZ€³?J›Ú£NP?_
ËJþ™Y?J›Ú£NP	4FGL J0451.8-4651?ÄÎå="ÆTÀCÀe¾ ºÀ9ßõ}ÅþÀ<A©n*@ü3öQ«n@ÿ#¶?¼¸ì"x?¹ªiJœ[k?ú|±|nX@¥CžNl¿æ‡¸Æ…Šï¿ã!'fw-^¿ç(èÁõÙ6¿ÝÉ%8HÇ¿ïþ˜÷³*d¿ïù|´†…AGNfsrqPKS 0450-469?ïÿTK²û–?ÀÛµ¯?v‰ à?ÀÛµ¯ƒ?ïýz¡DÖ·?QÿÍm%¯Y?4*õÙJF}?QÿÍm%¯T?ïÉã?™©8XU?{vžu®}å?™©8XU?ïÿ}Ak×?êï	·BÀ?WҟÅ.Ô?êï	·A¯4FGL J0451.8+5721?î$Y ´›¨@ £úLaØbÀ:ã9º5ñTÀ<{‡(}Î@!³§ú/†€?øR7y…?Ó4ÖÁ˜;K?ØCP·¨xZ@óݗö+k@¡vÈ3_ÿ¿ÐO¯j¼6}¿ïÿèþ†®/?ïý›6QË¥¿Ôný?¿Ò÷si"(¿ë°Ú=x±mAGNbcu3FGL J0451.7+5722NVSS J045148+572139?ïßZg·.m?¬ÇòJÙ#Ö?pRÌ$hÉ£?¬ÇòJÙ#Ö?ïö xchœ?jx‰–t?R¿9.Å+?jx‰–t?ï¤hfŸC?…ã=¥ú?†åæX/<F?…ã=¥þ?ï³z ±ÞÈ?x§#…'¡à?ƒ!wӈMó?x§#…'¡á4FGL J0452.0+2100¿ê<Zß±À,ø§ayWÀ;YzŒŽ\À<…ñÓ'é@"³Öe|Üu?ùQÉ÷/væ?Ï+=…òrÏ?¿!%¿'6|?òkÓyq@sœ§Àù°¿îÂÉ.4¿î²;QæM?ïÿXÛch…?ÝÇ×DŸí¿ã¥u«?q7k¸FFAGNbcu1RXS J045214.8+210307?ïþü6>ˆN?¿V
¸ ? <œ{Y?¿V
¸˜?ïþp€‡•?Qò€sô{?.X÷÷†Á5?Qò€sô|?ïì–Y*i?p•ê¯ªæ?ci¦Õ–ö)?p•ê¯ªð?ïõ®u(A2?Lûäî¦VÒ?T£¯}žD?Lûäî¦Vé4FGL J0453.1-2806¿î-¼§c¦1ÀB"Â	$lÀ8'Îï¼»ÞÀ<©@։å@A|wð@P­Í-DÝ?£¡?Ö.ËE?¸ªÀ³cð@¼Ý!®¦q@ùÃOöb¿ÖE»ámÛ¿äêB‹@¿èô¾þØㆿê"úÞ­õÇ¿ëù÷2ú(¿ïÿÓÀíAGNfsrq3FGL J0453.2-2808PKS 0451-28?ïÿF™y?$ßùò¹`?0ÐÖÃ?$ßùò¹I?ïúß_@Î%?Vj£3!"?D''üÇoö?Vj£3!Š?ï­/k¶Ôã?ƒèbMw¸Ã?"´%Jǹ?ƒèbMw¸¿?ïý(ñ‹8™?,]ÀdÑZ`?6¸s¦;@k?,]ÀdÑZ:4FGL J0453.1+6322¿ÕڂËF@(V|ᛑÀ:S±E‡ÊÀ<+¯BxJ"@ ¦ˆgB.@zlãX)?ÁJº"üq?›-¹ÌƒÁ?Ýú$Á‡@émÇXÅ?í£J¨š¾¿çðÇþ±Ì@¿èú)(î6¿ÑËaè¨K¿ä!æ­j1¿à@"°%ÍAGNbll3FGL J0453.2+6321NVSS J045312+632117?ïû©'Q?:–‡N*ŒC?AY»÷–º?:–‡N*Œf?ïü`/ä®Ï?[xûuÄȎ?<þ€Ú‰"à?[xûuÄȐ?ïô'Ñi?ec'ãö^?W°]Ñß/ã?ec'ãöI?ïæ6†ÕÉ?U¼ð×g?iÉùy*7ð?U¼ð×j4FGL J0455.7-4617?é"o'ÂuÀCi˜áõ²À9
¥ÿ©þÀ;ðšrÝm.@&¢†}20@ÝÓ4ÅÚj?§!­¤¾e×?´âÎì·£Æ@	ÿG¶@yX«gÍ¿¿ì 	·¿ä±Ö;áWž¿ç¥c¯˜	¿çWìPÓ¿èŒYÙ¿çƒO
)N®AGNfsrq3FGL J0455.7-4617PKS 0454-46?ïýOçþ>]?-±3"̇?5€À
q?-±3"Ìt?ïý!En?QoÊ#{©û?6÷}ԏ–7?QoÊ#{©û?ïº(ïó?yK†®l±í?uÄ9ƒ;þ?yK†®l±á?ïü¸nî¶d?,PŒµ33?:<ˆŠLáþ?,PŒµ3,4FGL J0456.2+2702?ë0´Ö—/À$0H@áÀ9µ~q'
À; Œ‰ޚ@•tÁrüw@ïÇ£˜ ?¼xtŸ¨ì?Æ.ëzâÊ:@£É%x_@ phó´m?çÜ"N‰{¿Ü^d¤ÅFÇ¿ãc3vO¶¿æu
þÆD¿èå@6&¿ïÿ¯b® èAGNbcu3FGL J0456.3+2702MG2 J045613+2702?ïÀJ4ïº?~DN ÕˆN?ûÚåˆ"Ï?~DN ÕˆL?ïúbXw‰ž?dqŽÁ¢Õ?Fvž!يá?dqŽÁ¢Ö?îòHT?ìÿt½â¨?¯Ž—àÛzÒ?ìÿt½â¨?ïÊeín™›?dC%œÍ?zÍ	H³2%?dC%œÏ4FGL J0456.3-1634¿ä"b›YÞÀ@^JÀ:Ý'nâlÀ<›×5Ü@ÎFtƒ‹?ü½úºpª?Ð
]O¼V?Òrsºâ¿}@‹G&/>²@ÃU¶ÀÆÚ?チ_æðe¿Þ51e'Ìù¿Û§Î›Ya¿Ó)<ÅS¿èÙÊÁÚ«]¿áœ]=ó«‰AGNbcuNVSS J045618-163552?ïÝÂÉT'/?p–]­¤6—?q›Uìh?p–]­¤6"?ïö-Àc?iG3êJ?Só¤ÿ<ç?iG3êI?îy¤I<å ?†_M?¨e»l1¦?†_K?ï;¾I~ˆh?€òûVÿ?˜ˆ6Ð.òò?€òûVÿ4FGL J0456.4-4043?ï•4•‹ÁŽÀC:-ƒÆÉ~À;oºzº±AÀ<ËÆ+ÈÛ§@úu.«9)@ü!ƒÞFr?ÅEÅÇtô¿±Tÿ5Õ¥?élґ1ì@ý½Èäá¿å3!€nÅ¿ìé ¹³ë¿ÞžOv_Ø®¿ÚMõÏ¥¿êkŒÞl²?ËÞ3<ˆ]AGNbcuPMN J0456-4041?ïýÆÜþ?/¹Òºã~?3ñϙ<?/¹Òºã"?ïþb<$éz?Hñ•'1HA?)Ü=±h^‰?Hñ•'1H2?ïÃyMŒº?€ÿžu?~CY9ÿ¢¼?€ÿžu?ïþªÙ¦Îä?vˆInË?%Re"¼æ?vˆIn¿4FGL J0456.6-3136?á 5!lÐÀB‹;BÌ-kÀ9×Þuk¼çÀ<}'Õ1@êÅÝð@¥qŽ¸•?´8=´›É?µ8æÒÝ]?ùô3xÓPu@Q/¹¬²?×Îÿ¬óéq¿á­w!t™Û¿çøÃ*Œ›"¿æm¾ÌeŸ¿ê½ÁÆßM¿ïÿ°_ïÉAGNfsrq3FGL J0456.3-3131PMN J0456-3135?ïúbò£¶"?C€¡Tž?Ft5q%«û?C€¡T¯?ïöo"xoU?n_¬Ü)B?S ×!WÁ?n_¬Ü)B?ïÙ8S&8E?vO°—aÆö?scÖlãÝ?vO°—aÆö?ï¼¹Õš?o*òƒ¤…Š?€ÑŠ¿:Ç?o*òƒ¤…ˆ4FGL J0457.0+0646¿àq0w­À5«Þ灃ùÀ:­¸4TÀ<ùÅS[È@/©RtA@¯U!š"?Á­‹¾åƒ}?ºF6mÐ=?ô—'ML¹í@ç~­Úï$?åïB]r¡Þ¿ÜK"]xB¿æ韀äA¿éå.X•¿éO€pÓ¨¿ïþcèݤ‹AGNfsrq3FGL J0457.0+06434C +06.21?ïû¡ñÄÕJ?@!ü[¡Ýæ?Ax8ìªÙr?@!ü[¡ÝÛ?ïþ-Œ{*©?Fáž*4
Þ?-'8MUu6?Fáž*4
ó?ï<GH?…ë¾?‹ðýî­¿?…ë¾?ïûÉìdÍ?/º½ Ç&??@ØOúlÊQ?/º½ Ç&~4FGL J0457.0-2324¿éVXÔJÁÏÀAs;÷'À6q%»{k±À:øu/@­!­ú¤¡@ξú|2?€a—Ó#‡?³YéA¢@*x®I#`@ ȋ÷o¬¿Æ律4ë¿ß3âÂ\†¿ä~!nÑ¿ã¥cœ‡Š£¿ç{4ßZÃñ¿é@|ÇÑ»IAGNFSRQ3FGL J0457.0-2324PKS 0454-234?ïõ²èe?OÔwX©‰J?Tš/5×Ã"?OÔwX©‰K?ï™--g՗?¥¿Hïó‰?‰´´¦
š?¥¿Hïó‰?ï…Ô>¨d?ô½›"áâ?ŽŠðUç:?ô½›"áà?ï";}¾º?‡÷{Z^?Šñ> Qž?‡÷{Z]4FGL J0458.0+1152?ïWF"å¡DÀ2¦šíV°À:îê'ò#À<R1Xg @!ǎàV?ýÛRUÆÜ?̈́`¢W-c?™8 °d?¾žœ7ً!@-TÔî"X¿È¬Ãœã%¿ëÁ!h/"B¿ëÍÌsáy?Òó½‰bë¿á‡¦RÁ¿ÎÿùŸé"ÚAGNbcuNVSS J045804+115142?ïÿ7{½Ý?Ñ Ò
ü®?ˆD`"5?Ñ Ò
ûõ?ïý}qa>?Q 9ëMþó?7<töÊ?Q 9ëMþÿ?ïì@ÍÖ?hkcBàAò?cä¿2)â'?hkcBàAí?ïóz3†Ã?NïU.ù…?Yߘòx
?NïU.ù—4FGL J0459.4+1921?ïÔ5¼öÀ, æ)•$ÀÀ;"ù÷¨À<BŠgÍn³@!ë‹Ô´ù@!Mø±W&?ÎM/Ége?‰régÉN#?À&¯X‡@l5%Ñ¡¿µ@cÖ>;?Û7½;_QŸ¿î˜Ù`ð?ßgk^Å"¿Õ;ˈ).Í¿å@¿ã°>AGNbcu1RXS J045931.5+192242?ïþÙÄW?/øÜ5žl?/oú"ô?/øÜ5ži?ïþ"œ¬?CO»'?<?&¾Ö>õ5	?CO»'?X?ïÖ³…Ü;è?x­àé¤K?t¦=â
&?x­àé¤K?ïý@[¤?-)Ó °?5ÿ]'ÒßB?-)Ó •4FGL J0500.1+5447¿ïùúÉÜ@'r%·I®À:žÆ3¡îÀ<,©ã"¸¯@Ƃe n@±Âþñ´?Înø†9?À±½½:]Ÿ?í=Àgc¼@Y9Ô1<¿ïÊô Pm?ïºiúÊ¿èín˜dt?²òpËD7¿ïÿø]ˆò?ïþ÷ýÖÛAGNbcuGB6 J0459+5441?ïٔÓ[ì©?'ý"ƒÖ7o?s5–R	«¸?'ý"ƒÖ7q?ïÌ+zŽX/?ž™)Qƒùg?yêB¸Óé"?ž™)Qƒùf?ï'Ґ¢?"_¿	ó%Z?ŸžmÅ­ë»?"_¿	ó%\?ï¥Iõá‰H?Ä->ä©Z?†­'‡®?Ä->ä©]4FGL J0500.2+5237?¿–a¯yÂÏ@fL¡™B\À9ÖI°M:EÀ<ïH!×Á@!\$˜Ö¸?þŒý"$½?³ÇÝ_þ(¡¿'¸îª_å?߅&šôb"@-Ÿ¿ÛÓCÁð?ïò¥­Û¿è]¶Šk¿Ý– 7˜s¿×^ÎA–ù+¿ËŸ¥aÎÒAGNbcu3FGL J0500.3+5237GB6 J0500+5238?ï߀-ë®*?hGLÅ© ?p?é
(ëp?hGLÅ© ?ïôwAÅá?r0)¼$:?W|t=?r0)¼$:?ﱅÞ"œ
?'[Šëí%‹?ƒžˆwXý{?'[Šëí%…?ïnN›´À¯?''øP¦?'6,‰gê/?''øP¥4FGL J0500.6-4911¿ÖÑø´~ÀBý@=ݱ!À:­Ž!–R½À<Ÿù¬ÿ§ë@ [»=XP#?ürùà0W?À5AU_ØÙ?¨äEdc+ô?ì¨OÌû@Ø×¾˜V£¿ïEFáeá?ïÒÖ0ù¿àFÀ¾Ìƒý¿Õ0ÀRŽ¿Ý"¡}=ÃZ¿ã•[$AGNbllPMN J0500-4912?ïÿ‹"EäÅ?Â.u?
î†Î¾?Â.ÿŠ?ïýˆ4:«Ú?Ví¯Þ|ű?3¾^*¡2¾?Ví¯Þ|Ŧ?ïõ¾Í]¤9?`§0é3äo?T'eD·Œp?`§0é3äp?ïûԊ‡W?6+Û±ƒ?CÌ­Õâ¤-?6+Û±[4FGL J0501.0+2424¿ãâÏÉtšÀ%Š|àü.ºÀ:à{ö£ðÀ<_c>"¹†@!W¯K‡'Ü?üÄ<"¸?̒üÇf[?Îìì¥@°ý¤?÷éä4È^©¿ïÿôA…ÜM¿ïï&"è±?ïÿü9¡â=¿Égâ<u§¿âð!愯¿Öv"œ;AGNbcu1RXS J050107.1+242318?ïø4"M?P'O®fS?O,õ³šÉˆ?P'O®fQ?ïs˜×47?²H·‹S?'Œåy ?²H·‹S?ïWŽLDF?Ž7­ƒÛl?•Î6ww<?Ž7­ƒÛl?í"-|˜˜(?¢áÿØ|j2?³Þ";>¾?¢áÿØ|j24FGL J0501.2-0158?íÂ"./¥À9J]ž@ÈGÀ7­†!ÐýÀ;íZQ@x…v!@$Q2øzÑ?–Ö+Ú¤Q?¶"À%@ϼ¡Ÿ@‹F¿Å¿Êɹà<¿âl•õ *­¿å©Æؗk¿åFC¡+¿êңܺî¿ïÿ½ÅGóAGNfsrq3FGL J0501.2-0157S3 0458-02?ïõ@úX'?PðmbÑá¿?UÔNÞO?PðmbÑá°?ïòì#a?j.WTv:
?[ïø'¹=‹?j.WTv:?ﬢ%7D?"?#JvÄÚ?"×v¸ò/A?"?#JvÄÝ?ïûÛ¸5?68֚ï#^?Cä'Ï)ð?68֚ï#"4FGL J0501.7+3048¿îŽóðGEÀ@eށ*7À:hÚà‹ÆrÀ<¼²£UÛ@!aB|§E@	ý¯Ã¨?¾!°¿Pˆ¿¤¬Ž¾Ê*±?äõé@ Ú?ý÷þyX1?¸Öf~'%?ïËKøüր¿çKlD̸«¿ái%}½ðç¿ÛÀ-Ëë%¿ÌæFÆbûMAGNbcu3FGL J0501.8+3046GB6 J0501+3048?ïåg_H?h=ôe^?jà€˜ ·Ç?h=ôeb?ïâï:?-?'öêGòq?mÅâÀÑâ?'öêGòq?ï·´a»ÿº?ä4»ÃAÍ?'ç'p?ä4»ÃAË?îœ%GZhÅ?"QÙû¥Å¯?¦=«ŠYs¢?"QÙû¥Å®4FGL J0502.4+0609?æóöªÇšÀ4Ü
Ð=š•À9ÌTæ³^À;¼Ñy÷Ü@:꘺¡|@jŸ±
Ï?¿Ô‡×$i—?•[ÂéZ]?ÒØöî‡@çzÊÒ!¿Ø¿o˜¿ä˜±<MŽ(¿é"ø!å-¿åG†§NŽ¿î"6©	y&?Þh!Q‰`AGNfsrq3FGL J0502.5+0612PKS 0459+060?ïø7³X?JÿMn_È?O!3Ÿ´ƒ?JÿMn_"?ïþèˍÛk?<bMÓ_<†?!sG"IT‡?<bMÓ_<v?ï^êQH?ƒ‰@$²ç?ˆ¨Ek¿n?ƒ‰@$²å?ïþµR®?%2¤ª¾¾?.ÔªÕÖý?%2¤ª¾À4FGL J0502.5+1340?Ü^qš7þªÀ0»)^ž	À:&=²èöÀ<0B½ê²@)û'êV@rÜ£Úe<?Á͒švä8?­Ê­¸µh­?뢱Èd@¶5?|푿²çgWÒú¹¿åœ|m8è¿ÝïU"qD¿ã%‡
¥Úð¿â<
½s=¿él¯áY¡²AGNbllPKS 0459+135?ïúfF9a)??ô| ºÆ?Ffç{^ƒ??ô| ºÆ)?ïþEÇW;?LŸNÇ?+£ŠŽ\F7?LŸNÃo?ïæ8]X?ta,˜òsw?iúÇý¢¨o?ta,˜òsr?ïõméê²þ?@𿋱?U$,*šÙ?@𿋱4FGL J0502.5+3438?ì<䗭ƞÀe©>ê!À8ïíO#SÂÀ;m·‹(U@¼"ŽðsE@‡z³$…?±1é\$™?À9×|©ñ@_;©#z@(ÿZ¾'w¿ÃžvãŒ+ó¿Þgö^k›/¿ãºÔ¢Y0É¿äÅÃù¿t¿é"´À;™ß¿ïù\wÐ6AGNbcu3FGL J0502.7+3438MG2 J050234+3436?ïâ­u*°‡?hÔNa!®V?mRŠÕOy?hÔNa!®X?ïù'gñ•?bMá®õŠ?I÷Î`9­H?bMá®õ†?î–úó6ýô?œLœðúX?¦P̐ ²?œLœðúY?ï±ôq¿ ?nϲÜ=ý9?ƒ'㐠?nϲÜ=ý>4FGL J0502.9+6533?çG=}¶	@,¢ÿm3	BÀ;B§½HËKÀ<¿]K4²@"<}ðÿ1?ú4ÉÖxG9?Îý"û|ã€?µG@†Wó\?íà8Ÿƒ¾f?ã£éõZ=A¿ïê¤N(ÿ¿ì-ã}"S¯?ïý©®º"¿à>qTÖò¿Ô;‰"%¿©æ"'ØäAGNbll3FGL J0503.5+65381E 0458.1+6530?ï½|¡µ†?´ý÷fÆuë?~¡A¯%<û?´ý÷fÆuë?ï­x?ö?¶gÿÌ?žŠPø?¶gÿÌ?ïäKMU?A?ppm'Pê¬?k´²ªÀ¾&?ppm'Pê¤?íð·	Âû?¨…Ä1r2À?·zG±è$?¨…Ä1r2À4FGL J0503.1-6045?ïø½YÀBG¼Â"çÀ:Ó^†žSÀ<4¾ÓåÅÂ@^Æ1Ó@.v]Tní?ÓÁ1ùwOÃ?ÙE~ð ç@`Ũ]_@†lQ÷?ïûŸíp±¿éq'Šˆ"ž¿èîwÂYV^¿è(¶½–Îä¿æsûŸóû»¿ïÿ.ÿqå¡AGNfsrqPKS 0503-608?ïù7Éîð»?a³¾gÄöý?K ØD=3?a³¾gÄ÷?î\ÌfGyV?»ºOӋLH?ª39›ˆj—?»ºOӋLH?í¡w?Àõˆ? üqÏ+©?²ôFøSÁ? üqÏ+ª?쥘àkt?¥6}æzû?ºÓ8ÿì¤e?¥6}æzû4FGL J0503.5-1116¿ë½ÔxªöÀ=âÅ\–À:˜Ä0FéÀ<id»k{y@ žMQü?ýHò'hûl?Ď:?ìÕ?¬
rIÉw®?æSò@#Ü~@'Ä{D™ã¿Ý'NÜÜåI¿ÜK(\ëhn¿ßÁí@	ÛK¿Ñ·üƏ›ê¿â=U–4ŠK¿Ôf%ƒ-ùAGNbll1RXS J050335.6-111504?ïýv"êÂC?)|Ê^j?4KX©íéO?)|Ê^iò?ïþ]üA½£?A‹wæúZ8?* ;ä%У?A‹wæúZ;?ïô‡OÆS?eDä·ë¸"?WÆñ`sYi?eDä·ë¸-?ïó"°¼³?H½B†¼ló?Yú؞†›ˆ?H½B†¼m4FGL J0503.6+4518?g"Nô]ŸÙ@ŸÁßeVÀ9¯Üöæ{ÊÀ;Üè,¤£¹@ ¹uj:[q?þ•i‰0–?¿â=ž4?»ïÒ Ì=Ü?ý2Ú}wØ@%™¼Úç¿ì¾²Ã6K?ÛS®=j™§¿ßväOö7¿Ú"¨~cÞ!¿âX>à»l'¿âì&ďçAGNbcu3FGL J0503.4+4522GB6 J0503+4517?ïé'̱Ã?l¢¥ÊêҐ?fn3ôN=å?l¢¥ÊêҐ?ï'ÀF3è?´#¡ÐŠ°?›÷9'ÿ'?´#¡ÐŠ¯?ï†öX¥ù?ŽօŸ ·?ŽB|éցu?ŽօŸ ¸?ïa±¾Q?Š•·;ñ€?ŸÓÉÈ?5Ê?Š•·;ñ€4FGL J0505.3+0459?è˜óòƒeÀ4Ü9ÿÖ•À7jD†AÎÀ;öÍ0 @ØF·õOM@'Ï] Å?•€RY#?»\•­%è@#VŽÅ*A@ÕhÀÞ­¿Ë*(][Œ¿àèû6l£—¿äüÒï%½)¿åÂψh﮿ëQþ'A·¿ïÿ±[W>«AGNfsrq3FGL J0505.3+0459PKS 0502+049?ïÝÿ1MÝ;?pQÕûE£r?qgYc?pQÕûE£q?ïÈÜû`ûâ?—Òä7¤ÝÌ?{''O'x?—Òä7¤ÝÍ?îHݒ>¡Ü? šÔàÐ?«r&ÜâB? šÔàÑ?ïìlÙ;O?]60?c"&Äå±?]6&4FGL J0505.6+0415?ÅðvCÀ50ɧ~^«À9Ì1p»SÿÀ<KŒÆL€@ ËE05ÒË?þÇë¼|?¼¦ÂÞ¼Š?¬.Eã?ï왡&UÕ@.	™Üµx?ïÒá锄¿áݳÍêÚ¿ä…™1"οÚ{$
¦\¿Ú;¼ïŠ¿âsÂóáAGNbll3FGL J0505.5+0416MG1 J050533+0415?ïôØc÷Y?M$•™jo?VOÝ8M¨?M$•™jt?ïú&
!¤:?aG"*C'7?Gg×yo–?aG"*C'8?ïÌÿ Ì?xù$ a¬?y€8sï™Å?xù$ a¬ˆ?ïxøÏx£k?y –Ê«ËÓ?àæ뒩?y –Ê«ËÏ4FGL J0505.6-1558¿ëg'Ð¥>À>n¾‰¬½À:"À';¯À<~iœ{Ì)@_ob¹]¯@MWoÈ?¿Ê™@Ù9?›¸œÇªÎ?ß¡'à'§b@šP¦`§`?ï'ɨU@¿áÉåX4¿ÜÉ þé7¿äæã>SLÙ¿Ô'üŸ"p¿äÂßäÆAGNbll3FGL J0505.5-1558TXS 0503-160?ïýû¨2¸?'/ëmR]?0"¾j?æ¿?'/ëmRž?ïþø Èr_?=Ÿ9]Föç? }óxÚ3?=Ÿ9]Föý?ïìxæªcù?s]š®ÆE?c‡Uœv?s]š®ÆD?ïü1'RT?-ÙÃÇäÎ??smm^æ?-ÙÃÇäÍÙ4FGL J0505.6+6405¿â$^à@x@+kJfUŸoÀ:Í*ÀêÀ< {ÃW@+î¼@žß(Ã?¸¤³~:ž?Ň>£(ä@`ì>'Ï@	m8?ï³ÅP˜¿Éü.dAs¿çôß:šˆ¿â[?î¿êŽ›~¡¿ézNW‹ØAGNbcuTXS 0500+640?ïzÍ"ðð?ˆ8fyÚ?¦[¡ðÑ?ˆ8fyÚ?ïøáåSËÄ?d³4›ÞI?Lxj°Ðð;?d³4›Þ@?í¯',ßÅ)?¡Ïìïô<½?²ƒv™Ö¾?¡Ïìïô<¼?ïü»	ÁL?,ìòàÀq?:'±õŸ`?,ìòàÀq4FGL J0505.8+3322¿Õ)õŸ
sÀGlãËÀ:f÷ù¡A.À<­-@ l"
qË?þÄØý\·'?ÈÝ5:I|÷?Èϐa³'?ýÛs©EH@â²_¤¿ïÿ	*K-%?ïþY¢2ÅO¿£Gt!©·¹¿æ^ú+ª¨¶¿Ò"Üޒȿíñcºº{'AGNbcu2MASX J05054288+3321355?ïv_,N+X?Ž7|@ŽÁS?'4v:•$?Ž7|@ŽÁR?ïå>tõiT? uw'Ž?jÁ‹
–ª? uw'Ž?íDº¿Ö(?§®xV?µÚ*KöÅ?§®xV?ïB3	›?‹€ÐFŠ@?w¾9žÌ›?‹€ÐFŠ@4FGL J0505.8-0419¿ïÁ‰ºmÀ9f?x»Ó€À9·iþ¡[/À<œüûhÂ@«uÄ'aÄ@Ä#°ß0?µcl6	&?›m=ù"\ò?ä\õ8ü Ð@…ìiJF?ïïNlta¿Ö"vÅTÉ¿ç9.ŠWw¿â¿üò¿ì)ÞJ΅?µmôÐ!AGNfsrq3FGL J0505.3-0422S3 0503-04?ïùZ•ê°ð?CŽM–+Ù?J•¨U<I:?CŽM–+Ö?ïÿ7Vsº?3±"AñÆï?<1ˆ×‡?3±"AñÆê?ï|ñwŸ9?‰Å Ý¥£Ö?aÜÜ?‰Å Ý¥£Ö?ïþ
¡•Ï?"-ü+U§È?/^%æ£	9?"-ü+U¨4FGL J0505.8-3817¿ïVmËT¦ÀB/@Ý?á—À:²'f™'À<ª; †ô@øáі¶?ÿ©òâáH?ÂâÍ)¾ë8?­#Ú¥¨p¢?ë)õœÏ®ÿ@	n»·¦Ÿç?ï¸Â‰|ëä¿ä"§Ös¿ä#ÁÛØ‹¿Ðð~BP1œ¿å¨Ñ F1¿ä3Û._"AGNbll1RXS J050559.9-382059?ïÿ…¢rR?cä±AñE?º—ck9{?cä±Aï"?ïþœv…þq?AÀ©ñ'¸?&8— ï¯?AÀ©ñ'·ö?ïûçÔtפ?GdŸ,ôÈ`?@`®,¡mþ?GdŸ,ôÈ>?ïûÅ%…'?+õ¢Hqœó?@ë¯ié¹^?+õ¢Hqœä4FGL J0506.0+6113¿½¹ñ0L÷–@(1\FRÀ9®ð©Jç…À<&¼ßï¿@@ ,µ?½Z@'.B2ªw?±"Ï?úT?Å^ïN­?àPž¨ø@Rïl_¿è'ýº*‰?¹SŠk©F`¿æ–!W=ª¿Ödéc±UM¿æ}º«bú¿ÁSæ.Ã7AGNbll3FGL J0505.9+6114RX J0505.9+6113?ïù›þõ?BS÷/É*?I+«Òt?BS÷/É?ïú5±zö¨?j|sAõɍ?G):%\—?j|sAõɏ?ïìæà'V?k$£{ôÝ?cómª?k$£{ôç?ïãIzˆ?]½ÈÏáÎ?l涅éxC?]½ÈÏáÒ4FGL J0506.0-0357c¿ïgёŸÀ9-DŽO¹À;{È0…ÙÉÀ<â¾|§ñK@  czΨD?þñìVuX?ÖÐ^ÚÖÑ?éµ°P•CÊ@
h¾/?ÿ-å^0´¿à­Îod;ê?ï"E¥%¾Ö?Í91d|'¿ßCµA?æJ¿ãð"aùð¿ïÿvä܎AGNbcu3FGL J0506.3-0357NVSS J050605-0401520?ì˵ox´È?´ S»ym&?¹¢T":YÉ?´ S»ym&?ç–ühŽK?Ñ1ý´<ˆf?ÐÓÄ.ãj?Ñ1ý´<ˆf?êÃoeâY³?²¢¿M`éŒ?ÄòBhv™2?²¢¿M`éŒ?Úò
5ã?¹d¢TF?âøúåxŽ?¹d¢TF4FGL J0506.7-0857¿ÁÑ$øfþ>À;O¯§"YÀ:3+y*ŽÀ<Y^¾Ò@"¾ì‡@Ÿ.cÀ™¹?¸3°ÜJÿƒûW2'?̦WB1(@/DŒ?ïÁ6á¾vs¿âØŸUd¿ây,Áÿê1¿å3+;-C¿ÞÚhH¿â¿ÚÖ­@•qlAGNbll2FGL J0506.5-09011WGA J0506.6-0857?ïù®4ãº?EÝ GÓ?IG§,q4?EÝ GÀ?ïþ'Šší?A¿Øâƒ*n?&×V^ñA¦?A¿Øâƒ*R?ïèîü_õ?rQy¸ÀeÕ?gø  ?rQy¸ÀeÝ?ïøi-åú®?:¸ØÃý
;?N[HhI?:¸ØÃý
4FGL J0506.9+0323¿ç9mþvöÀ5\ÓZ…‡"À:wO"¼
À<ZÀ2Š–Ç@ Ja·Õï¶?þÓۙï)ï?ÁÏo¹Ì?¤)JQ1öÈ?ãO]¶>–@Û̈́ؗ[¿è—¢KïÃ?ïé%=QD@¿ÛÈ*;<ìð¿âP7…¨K
¿ãJ™aj?Œ5¿28!AGNbll3FGL J0506.9+0321NVSS J050650+032401?ïö?(—?PŽÕUô9I?Só®ÑåZ?PŽÕUô9]?ïûîOk`?lÔj²Ì?C€FÂR…)?lÔj²Ê?ïÕUæ—i?xB_ê`êÒ?uU´K0ê?xB_ê`êÌ?ïÂjDáì…?n™£N.í?~Êݏ	¾K?n™£N.í4FGL J0506.9-5435?¹å ³HÀBb‰üm¤HÀ9·zn['nÀ<D€bï@ }ëišù@?öb¼'«A?¸p°íOF?ÁÃÆé³ãG@ýöÀ¼R@èWº§¿ê°Öâz^¿Ó³(¶ØnÁ¿É1£:৿ÇLíCÌ¼¿ÕH[¬¿Õ<{ÜDdAGNbll3FGL J0506.9-54351ES 0505-546?ïê"BkY?iuÙRë²?eݽ"¦øè?iuÙRë®?ïø×åÂbö?d[áŊY?L höt$?d[áŊX?ï‹)õt#?‹Ê	_žá?5'¢÷<?‹Ê	_žÛ?ïÔ6&Á?cBm«¾¿?uäìôs­?cBm«¾Á4FGL J0507.4-3346¿ß#0Ÿ0ŒNÀA¦
á'6À:˜CÖ¥éÀ<'">iƒ@ ÈôíÓ,¸?ü¸<ÿ?½
uyÔ­A?å›G;]?ÓwE|Y@ãòóýé$¿îY»È˜Š¦?Ñ*²Æ'Ii¿ÚˆüéJ1¿Þf*]㋿ÐGòká%¿Õ¯?ˆ¬ŒAGNbcu1RXS J050727.6-334628?ïû"àÔû÷?B\/DF©?Ct|¬".?B\/DFš?ïþýu'?L}ˆHÒJ??.Ð(¯wè0?L}ˆHÒJS?ïë<~€·?oÄ%F?dÁHoÒ?oÄ%0?ïù(Æ}´?=C3ÌëœÔ?K\çÂ	'&?=C3Ì뜷4FGL J0507.7-6104?îúǺNÅ~ÀAû‰?¯BxÀ9Ry§‹Ê¤À<¡V&}B@Ä*m @ö‡{‰ä?°ÅÜ~ײ•?²=Âno@@}ü…!=@ü!3Vn¢¿âMQâ É¿âò#žjº¿ç¤Ç+£¿åíuÿ‹í¿è˜b—¤ÌÔ¿ïÿÅ}M2¹AGNfsrq3FGL J0507.1-6102PMN J0507-6104?ïýûqÅVd?,÷"X¯)?0$qÕLä½?,÷"X®ò?ïýÃEÚ?H`Šg¢kz?1åק‰-Ü?H`Šg¢k?ïÏcÎBW?uãԔ·Æ?xqÎÞÔ\?uãԔ·Ê?ïôŽ)ûì=?IðzÅí(?Vã¬'…m?IðzÅí$4FGL J0507.9+4647¿å•Ykñÿ"@vÊa¸¼À:	ÅDBO0À;I%Ü3@ú¦‡é˜à@á~4¹E?ÑÚØÞÓàg?ØÑÐAÌS*@准qž©@_Êe"Yi?£Pª"¹ús¿ã¹%¨05¿ä`‰þ#r¿éÿ}Ž¡¿ï÷x§±ŠQ¿ì)	ä…P6AGNbcuTXS 0503+466?ÛñT<÷N)?ˌüÅð?âUá"Xë?ˌüÅð?Ûïñ~¶£±?Òôp	^)(?â@¤®'?Òôp	^)(?Ù䘢ñ?¶þRŸî\\?ã
³®‡tý?¶þRŸî\\?åP_VÆ:R?°ËN-Z~Í?Õ_ARs‹^?°ËN-Z~Í4FGL J0507.9+6737?è*M±ÐÄ@/ÉèPðÀ8vÖFÉ-À;›òâáH@!Š¿¨X¤?øž¥Ýtº½?ŸL¬^ ÒÑ? qÇÿ™¹á@ÔæŸê%@áY¡±ì?ïy¼NÐG¬?']$É8¿ÚþÜÇÔ¿Ë`À	Dø-¿Ð'¦ÂÌÊWƒ_—±AGNbll3FGL J0508.0+67361ES 0502+675?ïýAfa?30h5"wè?5ó{ÌòZ?30h5"wó?ïôÀ^y«‡?n>-«•§?VC¨ñ?n>-«•«?ï‰äõµð¶?¢2Œj?†Â'ƒÒÎ?¢2Œn?ïëK€óÁ?VâàŠ–Ø?d´ü??VâàŠ–à4FGL J0508.2-1937?ëŠïßU–À?2×@ÄnÀ;*í"1{À<µrþ$]­@xC¬':×@åPäôá¿?Êú8À»Çl?ØHC{)ìã@C"¡@µÚ,†Æ®¿ïÝ7~ŽÒ?ïÔ£"`š¿àé.AÜÄ<¿åºðáÿäÒ¿íøwÀ«×4¿ïÿý±q&´AGNfsrq3FGL J0508.2-1936PMN J0508-1936?ï$×m³Ëo?£–'å…<?›eI†'ð?£–'å…<?îæ!æÌ?µ(+›¨?¡žŸ=á"G?µ(+›¨?èÊJÇ"2?°­}ɽŸ?ÌÖÔãw7ì?°­}ɽ ?ìïNÄLi?¥"Õìn?¸…aݜ°?¥"Õìn4FGL J0508.2+5211?íû ‹'a@5#ŸAyGÀ:ÀÞ­ŸàÛÀ<4p¿…¼m@ 
z?â@I´˜c9?Ō[ØîÄ?¨ÉÀ°3å?äù]ÿºŠÖ@mà0ù¥?é"ó1»cï?ïøø²<(¿Õð¡¾+IZ¿æ
gAؒ~¿ç®±Ž'å"?·ôƐó'ÄAGNbcuNVSS J050809+521256?ïôÇõË?Vö±á'$?VqÔiØP?Vö±á'$¦?ïõŸŽÈa ?y‰ðMXŽ?TÀâo<À&?y‰ðMX?ï¨ãÉè~?…PÃi¬Íâ?…Ç=
…àb?…PÃi¬Íè?ïº]ߤw?r@©_±$?hºÈâ¡?r@©_±$4FGL J0509.1+1943?â¨)ƒo,À'ý¼#1]pÀ:	ã<zڒÀ;Ÿæ·Yž@E	¬§@†'QúŸ?Ο¹ï$'?¸F7qÜ;U?èì&>ƒ@ícíbt¿êÁ¢Âi¿ÝXl¾U¼¿ècya•Ç'¿èêŒeÔp/¿ïû'Á^Á?ÐC	Ÿ»òŠAGNbcuTXS 0506+196?ïõU½B?Ò?_WHZtÄ?UT…{€^m?_WHZtË?ï¤='^µÂ?›
M}U?†ð›¨R©?›
M}T?ì՜Æ(ª?£˜]Âimª?¹SÏ溭?£˜]Âimª???y°¶œ>R?‰;ø°•?y°¶œ>W4FGL J0509.2+5550¿ïÎ"Á&x@"Ÿhß½jYÀ:.¶ÁȍÀ<~'­N@;2'D"@˜<ÿ?ÅùԂM͓?¿í½‡?ù7ýÒÿõ@<!í%?ÞþáEª¯¿×*&ʺϿå$u*Nˆ#¿ÜÞ硺Or¿ç¶?A´U¿ïþ±`à•'AGNbcuGB6 J0509+5546?ï6ü[óß?œ!¹!`4²?œY tƒò?œ!¹!`4²?ﻐxí‰?H5#€Ì%?ú!ĝ?H5#€Ì"?îê81Í1¬?šÚ&®Ýn?¡\|ã,å3?šÚ&®Ým?î°;\•G£?‰dAJ}T?¤üJ6«…ã?‰dAJ}T4FGL J0509.3-2917?áu…sÀ›ÜÀ@ïßã*dÀ;	üȽÀ<»ÃlѺr@ùeä@|ÍT¤?ǼƒDÃ~¿n$M$;—²?¬fóªNN?þ‰ð¯*%¿ì–ŸV¿ÑΗÝ×·¿æ
|?ì¿Þ;	ÛØ¿à8èê9Å¿ïó/lÕqAGNbcuNVSS J050927-291339?ï÷ȓ¡Qd?Jý
'=FÍ?Pnؽ]8w?Jý
'=F¸?ïóãAMç?~3ÌcžD?YÖ9}d3C?~3ÌcžI?ï¥Ócý®5?'<m){?†‹'"rÉ?'<m)y?ïîn²Ž?P¡øāø?a'ñàMs?P¡øāú4FGL J0509.4+1012¿îì"Ѻ÷ZÀ1>°ÙQ?ŽÀ9YµÂÅÀ;î:Ç|*ô@s·ìj÷Æ@×~¶ß%?³<ƒd?¹1¨C«{n@:$¾ü*@Š_[^?ïû‹[é4â¿àAR—M¿ædÊðSº'¿æ†Å~ð¡¿ç'uÞ©¿çBž
A¢bAGNfsrq3FGL J0509.3+1012PKS 0506+101?ïþSçϟ?$šš–­ñÕ?*ÎAƒ	t?$šš–­ñ©?ïûÓû®;M?W²32äÍ¿?@°GÆÿ?W²32ä;?ï¤Nå=PÛ?'mÛÕ`?†ìF°«Éa?'mÛÕ^?ïôD¦K?F€ø¶Â?Wv³ñiö?F€ø¶º4FGL J0509.4+0542?êP1–«(À3¡zÌNøŒÀ7K(û¡ÌnÀ:î
N@êÙð¡¾+?ÿîȺïT·?–~1xï?ªŸþ…+£@H×°´h@'í~<Q¿Á@WH'>V¿Û R›X`"¿âÚ>û=y¿ß,J
æ
¿å#ªß½s¿áͽ¸‡ÆAGNbll3FGL J0509.4+0541TXS 0506+056?ïþY¨Ž?,ŒÀÑ0§*?.Úo…wg?,ŒÀÑ0¦¾?ï÷öt¢¶?k'¶ÁÑ¢W?Qæº'}?k'¶ÁÑ¢Y?ïÀ
#Ñi?ƒ°d̳ˆÿ?ùn@K?ƒ°d̳ˆÿ?ïÿ­PXq4>þùQUŽº2?«éã²â>þùQUŽ¹Ç4FGL J0509.6+8425¿îA‰Å; B@8ŸB»früÀ:ö,ÂãÀ<‹2§òø±@Ö ‰ÍÉ¢@`ù$C¬'?Å^I·Y¿³árÌ%]?ìá¼]"Ùç@ËîX^¼?ïúwàŒGL¿ç³ï†¿é¯Pð³[â¿ãƁŽàØó¿ð?ðAGNbllS5 0454+84?ïö—Ô{qì?cRXMÃÛ?RÐW	'Ã?cRXMÃÙ?ïE¬4ý˜Ò?¶Z|¿ÛW
?—Jy`Lå§?¶Z|¿ÛW
?ïxp¾Óõ?†¾ùG±.°?ñî%Ÿ?†¾ùG±.®?ï¤/$öÌ?~(Kí)þl?†ô<vÂL¬?~(Kí)þr4FGL J0509.6-0402¿î!ké[À8k™¡ýjÀ:'Ò¬áÀ<ZÆã~¿ù@ &|'²wa@h_dêed?Áb¥üÿD™¿'=<Ÿ/?ÒïœePç¤@"‡®‹?ï÷z>Š¿ã8Õ3£›¿çdú Å‡ß¿Ö—-ƒ›Ö`¿ßÖ­3ªQ¿Þ³Ë>WS¤AGNbll3FGL J0509.7-04001H 0506-039?ïûqÁµÅê?@¥n%ˆºj?B8ù(èZ?@¥n%ˆºe?ïýOL4{]?\˜²OÜ¥x?5…ž\%´?\˜²OÜ¥o?ïóý‹uû?f
í=º&ð?XéÈ
&?f
í=º&ð?ïì"{–mj?Pz~Ž÷«ê?c{"i'–B?Pz~Ž÷«Û4FGL J0509.9-6417¿â"‹éŸÀA˜>}QÀ:N°÷"0|À<"ê"]ðv@ Eúأŗ?þ-Aª?µ¾ S¿ƒ'ëÆ&d?Ð`¼ÃÀ3·@	Ý
$¿á¨†Ò¸©¿ã·S½v¿à*®"Óa<¿Ù‹z‡…šß¿ÚoUã·J¿ÜM8'}sHAGNbcu3FGL J0509.7-6418RBS 0625?ïÿKziǼ?
žj®v?²Ç"?
žj®??ïþk1A¡a?I:üÉm.?)Lëåéè%?I:üÉm ?ïûšŒ_c?U{dڗÙó?A—ù΂u-?U{dڗÙî?ïþœVòÂ?˯Œ‰¡:?&:— ÓÚÿ?˯Œ‰ŸÚ4FGL J0510.0+1800¿êÈÛÞëÀ)p—AЅÀ7÷uôxãAÀ;F­)¬@žp•@­@ÅÂíP?žs_Yhj?·«#Ú¥¨q@]¢r†/@xkv›"?¡ˆeûÖ~¿às-õÐú¿âKL.¬»µ¿â']ÂS¿æâZh+b"¿ê½4D«+AGNfsrq3FGL J0510.0+1802PKS 0507+17?ïûe‹(KÃ?<Ë
¼–ä ?BiÓ^Ðõ^?<Ë
¼–ä?ïø04Ï]_?a:Hæ	—«?O?,ŠA?a:Hæ	—°?ï¦Ü½h3?†Ú"ÔAÇ®?†Hþ¥òÁ?†Ú"ÔAÇ®?ïÿ©'Æ1ù>ýµâ¨b]?¶s'r>ýµâ¨bc4FGL J0510.4-1809?å­>Zq"À>05z5PDÀ:¢ÏîÀ<œÀ<uªŠ'¥a@%ònZ@5ÚBU?DZ¼»‡«?ÀêB> ?ôE;ÞÓ_Ž@
åð¦p‹¿àsco;!>¿×!˜ r¼5¿èà<K	鎿çŸÌäu¿ãC‡^ƒ˜ü¿ïÿšÏúAGNbcuCRATES J051015.50-181227.8?ïü…ºÎ	?>çÏZ‹=h?;×*)·ï?>çÏZ‹=;?ïýúc[Џ?LŸÑåYÌ?0,å!{Œj?LŸÑåYÚ?ﺤJùIG?}c‡€ì¿?VíA­®v?}c‡€ì¼?ïúnK7uŽ?65°Š>[?FFÓ")Ȝ?65°Š=ï4FGL J0511.4-6804¿åX…àxúøÀA%×ý'w>À:Ï&رÝÀ<.šLGp@p¦d]þ@ºV€?U€?ÅãæÄŗN¿mÜ^y?¡'G=VM@'º¹Në ?ð¿èZ,fWѿ듦¹Ù«¿ß|"¦Ò¿ÒŒ\š4Ê¿ïø×aütAGNbcuPMN J0511-6806?ïÿB `††?¾¹-<|C?«óï/'?¾¹-<|j?ïÿ%-Œoö?7OpRRžÊ?ZNr7¾?7OpRRžÑ?ïÖ·)?vû/ñŸH?t¤k~xx¨?vû/ñŸF?ïýðÞc\Õ?"	1«SË?0yåZk?"	1«S'4FGL J0512.8+4041¿ïÿúfÎÜÿ?íJf@%ßãÀ9N™û¿(ŸÀ;Å(wŽ'@0—²Ž³@TZDïô?µØJÀ~Æì?©ÚˆÍ¢
?ñËÏÇSH@Ñá»Fg˜?É"üÚ0¹¿ç¡Ìþ¿á¹	ÁŸÈ¿åF]É^ٿ༰À&Ì¿ìaU_Ø؟AGNbcu3FGL J0512.9+4038B3 0509+406?ïõ.aˆMÙ?RO'"´??U£<ïdO"?RO'"´??ïÎKšÊ›?­"#êñ©?xÚ~²š±é?­"#êñ©?ïªØöŒ?"h[–MŠ¹?…|IÂ\û¯?"h[–MŠº?ïú†2x,ƒ?5÷äàñ*z?Eç6Mö@?5÷äàñ*z4FGL J0513.9-3746¿ï¼ÜôƒµÕÀA[¾<Q‡À:ûÏ[óEÝÀ<~>TÏe.@)aIñæ@>"DÎf*?ÕzOÇã?ÞóÞ>d>Ä?ü4E]c@3ÝKue?îñïÁ™gð¿ÂtlùÓk"¿å6Aü$¿ïÿî—ø¯ª?ïþ{¿ïÿ7Mt'AGNbllNVSS J051404-374607?ïó…ƒÕCQ?d¯@ð;@?XôøUy^¾?d¯@ð;>?ïú¾ÐÎE·?k¨è³5?E¼Æé&e?k¨è³5 ?ëôŒ\¼4Â?©nHþŽê?À-΍,ø?©nHþŽé?ïñÐσÏ?\hb.)çÅ?\^aúøcG?\hb.)çÆ4FGL J0514.5+6247¿èŠOY7ù@+š™0¾
íÀ:£>ºOò‡À<uÌÿøsD@µø/°@"EœÂC?ÂnʸöV3?»ñ'Ž»F?ú|ÌQ#ß@€ýêQ¿æj8î^
?ìšÏú¿äW­Ñ_Å¿ÜXGŸ{ÛÄ¿â^zd¿ãœg¿¬Ó³AGNbcuGB6 J0514+6244?ï÷ñ"—š"?RÆÐÄ
/h?PÖÐÊø?RÆÐÄ
/`?ïò{;À:^?ƒŒLH !??[	ˆ‹BÍ?ƒŒLH !>?ïØÃØR¥é?~''Ð?sžÖ­
î?~''×?ï'n%¿è?j™ÜIAw¶?};m ±§?j™ÜIAw¹4FGL J0515.5-0125¿ÆÔv-ŸÀ5â]B¡À:š¶ŽœæUÀ<^@îݘÍ@s–ñ?ùüÜÊpÑú?ÔKa}H€!?Ô.á_+Â?þl˜å>³š@‹ö~•?ïû¢}˜Ý¿è¯L¾õsµ¿á§?¿³‰°¿ÒÇÜ£¦¿åŽé<o¿æÞÛB0|AGNbcu3FGL J0515.5-0123NVSS J051536-012427?ïøç
+Õ?TU%þþ7f?OÀc×P­7?TU%þþ7c?ïüÄ‡v»?Uã澛¢"?9ߛÄJ*#?Uã澛¢Š?ï:N¿´0¢?•\¬j̝?˜¶(	yëæ?•\¬j̝?ïÃN%Áþ2?fÝ©ß2x?~Xíç–?fÝ©ß2q4FGL J0515.6-4556?íeQn®7ÀA°K	éÎÀ8Äb\ìj!À;ý'æ÷ñ@ƒ)[Cµ@%AÁÇ?§´Èbô…½?©»Ôàu(Õ@$x]ï"@ØëpR#?!HW»0¿áÜ_|gY«¿æL8½¶¯¿äR½ú¡ò¿éwomv% ¿ëQ­DqIAGNfsrq3FGL J0515.3-4557PKS 0514-459?ïûÐ gNH?7¿æ˜Û
?@¿~bÆܬ?7¿æ˜ÚÚ?ïþ1F‰ÔÙ?Eê2-R?,ë—b²Vm?Eê2-i?ïÀÇ=@Ê?^oƒÞ|b?œ|á_›)?^oƒÞ|a?ïÿòô‰Œ>Õ¦ôT­jÈ>Ûöì呞>Õ¦ôT­si4FGL J0515.8+1527?æ;‰Ö¹êÀ*!ÅXdEÀ8ådÍßòCÀ;¶_"ÊÕ|@ É®ŠA?ýµØy©9J?®èO_8Ê¢?´ß="u@ÇiÃèø|@
¸÷f©WR¿ç8ôõ
¿Ø¨ÆÞ \A¿Øc¾ÁF[Ú¿ÝbßÆú{¿áÚaàŨ¿×¥Â¼þx–AGNbll3FGL J0515.8+1526GB6 J0515+1527?ïý;…Þ?0°J§ætÍ?6#Óáq?0°J§æt¬?ïúö-àÏ?\þOÔDt?D'›H|Ç"?\þOÔDo?ïؘ¸ä?zExäßÛ!?s³£÷9[?zExäßÛ?ïàÐOËW€?`È^%ì|V?o/°4¨~÷?`È^%ì|]4FGL J0515.9+0537¿€–=¶†ñ÷À2Iâ%úeŒÀ:÷ÒîNý"À<AÍ¡Þâ@Sõ±G‹/@'l6Kì?ÓaŽºú½¿",ß5N?ÂgBÚE0a?û»‡ëqR©¿å;66ó²¿å_"û-¿ã4íþÖ	¿àŸ=è˜Û.¿ã€´ÆEÊ¿ïê¶YFmAGNbcuTXS 0513+054?ïù$£ÐÑ?Hó3?Øä?KmqÀ¼¶°?Hó3?Øè?ïéªwvÐá?Tõßk÷X?fUˆ‰/ƒ?Tõßk÷Y?ï²AŸ…®Õ?'hATãM?ƒo˜"K?'hATãP?ïЦ0rîL?czDúÑ??w¬çƈÚh?czDúÑA4FGL J0516.1-7240?Ó|T…Õý•À@kè^9qÀ:gÝDUGÀ<2Ô\.Õ@|<uQ:Û@ü
éÿ
?Ãw©Å5Ô£?³'Þ
øø?ðG™ò"í?þ.zœ~Ph¿â5N`¶#=¿çv-NäH¿ç|U†DR?¿è@¦¹<Í¿ïÉéÍ³}¿ï	AÈ!laAGNbcuPKS 0517-726?ï×î鏵?rüÐ_I®Y?t‹8%sö?rüÐ_I®Z?ïI@x
Š?¨ãÄ»³?–×ðþ®¼g?¨ãÄ»³?ïM
Ï0}	?Ë·ÑkÍC?–^¦ð_?Ë·ÑkÍA?î9˜¶«íû?—/2 ·è?¬ft•A D?—/2 ·è4FGL J0516.4+7350?í~"$—7Ù@3Åf'|EÌÀ:~…AÀ<uV=ú6'@ I«w?ü΍+Í
d?¶{iضºè?°õØ^ÑF¯?ù-6´Çó?øòuJ×?ïÿ2z¦K¿çiÊ¿+y€¿Ï¡ªŠ,¿¿Ü=›{?¼¿Ý ¡€mΐ¿àÚÞrç~)AGNbll3FGL J0516.3+7351GB6 J0516+7350?ïú
-óËM?GËÂ|äÄ/?GËH0ÒÈ?GËÂ|äÄ@?î"hHüÛÒ?·6¼vƨ¬?¦É{p2BÐ?·6¼vƨ­?ïʝ×x©'?}G«Âf?z±C«>µ?}G«Âc?ì"õ-­çâ?£ä'×O?¾èV'Àö?£ä'×P4FGL J0516.7-6207?Í y&šGFÀAaÅ.rÚÀ8šq
"=À;Àâf'@·ut@Ù ¡`7?¢[_LA?¨'K‰Á4@!Àoz@h²ŠMÈ?àÀgc¼gû¿ß}¡ku¿ãŽ¶aP|ð¿à˜ö«:¬¿æ䁦ާ¿åó
ƒç€­AGNbll3FGL J0516.7-6207PKS 0516-621?ïýÆO5£î?)…J²Læ2?1͆Rà˜?)…J²Låï?ïü)ê
t¯?U³îÄÚë?>°¯¬ZŽ<?U³îÄÚï?ïÞ0ñqTF?r"y4ܹ?pç‡GUÝd?r"y4ܱ?ïþÞÛJ?2‡qǤu?"O¾»_®?2‡qǤ^4FGL J0516.8-0509?æRʊ?nÀ7YfYÑ,®À:`œøÉ«À;÷À¬-@ÆÎi/œ@C¼Œã©?ÇÝCýÛ¸x?Ù)x¸.@H/yjO)@	†qÀ?ÆxÌ$ý»¿ãu"FK=ì¿ê{>º¥Ù¿îÞwëÉè¿ïÿ¤?åÉ?æ2ËŸAGNbcuPMN J0517-0520?ïæÊTBû×?rI'lT_?i5«½(ó?rI'lT\?îæà6~;?¶Û¾(1?¡'ü˜$?¶Û¾(1?ì*æMC?©XÇÙKþ?¾¯PÏ%•å?©XÇÙK?ï	—ýj¨˜?ŽòO&?žÍRªí?ŽòO&4FGL J0517.5+0858?×)úVû&À01w…r›(À;e DC%ïÀ<ì&qƒÐÚ@!F€ÞaÊ ?ý痾Ή?Û
úD5ë?ïÿÜ>Y×ã@ÝK 'ß@M T3^¿évá]ÓoÔ¿îí0º²îÕ?àÖýr‡?¹¸ÁÝõ-¿ê²÷¤ëá¿ï÷ÇLZK¦AGNfsrq3FGL J0517.5+0902PMN J0517+0858?î~é«ö?©Þ)#qÃ?§áe@°?©Þ)#qÃ?êN­qº3È?Ð$ÍU©@Z?ÆÅJ90á?Ð$ÍU©@Z?ë
ýý6?±i	}B=&?ÃÔ'LJ?±i	}B='?åؒŒS?Àm'-ž—Á?ÔNÚæßYù?Àm'-ž—À4FGL J0517.7-1758?÷'¥À<ƒ…@FA-À;SPßìdÀ<n"d¦rÆ@ÙZ.Ÿ¦@?û˜'3?ÓààHŠ?èö'¤‰·¤@
;&wºL@JE)B¿àÔMà½?½t˜j¾e¿ã«Þj®õ¿îwàmò¿³Ï?Bàû-¿ïÿÂ"NßaAGNbcuPMN J0517-1756?ïÍw¡L?"K³ü˜N?y~ñÄ/YÌ?"K³ü˜P?拏ÛqC?ª¬L¬Œ?†™>I#¯\?ª¬L¬Œ?규hÓb?®SÙE«'?Å!Ž\³¶v?®SÙE«"?ï?H°míç?¯/<,e?˜éòBC?¯/<,e4FGL J0519.0+0851?äZ6³EÞÀ/ß-@ªëÀ9:2áԛÎÀ; ˆp|iÞ@ûPæ¢`è@Œz¤áÌ8?¹óô®é?Éme^(ªC@h@µKü­»?Ез=¿áIéXÎG¿èÐn**¿èƇ~9ö¿íÕç]qË?¤7ÀvõAGNbcu3FGL J0519.5+0852TXS 0516+087?Ù/#Uf E?ÈàÕ»ð8?ãhnUL¯Ý?ÈàÕ»ð9?àD|N‹á?Óãªd-#Š?ßwÕbè>?Óãªd-#Š?âÑ{ÔbW
?·Üؽ`
?Ú]W;Që?·Üؽ`?çk´O묭?±ýòu?Ñ(—`(¦¦?±ýòu4FGL J0519.6+2744¿×ô 
ýÀÍW¼w¯À:œŒ" ÚÀ;ætxwàâ@  àBöIÉ?ë6™ŸxÖ«?éýáí›N?æ‰=–c"4?ü"§—‰!@ùQê™¿æT~<Fl¿êöDà"º¿ä)%}½ðç¿Ôr;†¾Ì¿á$ùê<I\¿ïþ«6z'AGNbcu3FGL J0519.3+27464C +27.15?ïßì-úKU?yPè+åúu?p	éÚTÍ?yPè+åúr?ïþ|«¶?JS´Z©ñ?(5Dž÷u?JS´Z©ï?íýYp²?¥òÙÐô??·ð3"z€?¥òÙÐô@?ïú­rd~è?A^@ab©?EJ6n`(?A^@abÒ4FGL J0519.6-4544?ï4˜HÍ"åÀAUa=1¹¶À:6Ô;VdÀ<~¡ÆŽÅ@QmPæL{@'@œ¨AÓ?·óTKâÿª¾ÜŸ'Íú?ò•ôÿý²?ÿÓqíLa¿ÞÍ–%œ¿éŠŸ䍿æwé`J¿åÌQ¢_¿å4јäh¿ÕV¢ƒÎTAGNrdg3FGL J0519.2-4542Pictor A?ïë".»6?]ãW!ÔÞ?dlÑDÉqV?]ãW!ÔÞ/?ïÂe+¤Ý?";3u
?~Íj-'u	?";3u
Œ?ïv¨Ëp?ˆÖ5̈́¢?'*æŸ<qÒ?ˆÖ5̈́¢?ïgBôd?€«X1ñ¾f?"¼a}·?€«X1ñ¾f4FGL J0521.3-1734?íû[Øuè*À;Ž~bÜn+À:dál—À<>'(ŒD@¢ÁÙ©ª@É%x_?Á¡??Ûã?ϘiƒQX¸@
Ь¥åØ7?÷\mܧ`W?í´5&Rz ¿¸º¦?Öjì¿å~SEÎ@¿å->â"Þo¿ïÈÇ.¥/¿ïýD™`AGNfsrq3FGL J0521.4-1740TXS 0519-176?ϗ
曎Í?Ævñ‹fð??è=FYM?Ævñ‹fð??áÖ¶]¢E?ÖCÇ {Þ~?ÜSГD»u?ÖCÇ {Þ~?ÙI«¾F'ï?ºLJé1?ã[* Üì	?ºLJé1?Ê4ûe?¯ šñ4ý?éx2û{A&?¯ šñ4ý4FGL J0521.6+0103?ï2êÿÞåÀ3Zº8u'SÀ:ŽbwÄ\¼À<]Ú{9@ IKèá«V?ÿÉÉã
?ÀSÒ:
²?–8…‹"f?Ùât¿D£ô@$3"¸¿ï㸌íº?ïÿº*2Ùq¿åò³{Âîý¿ßEœVã;¤¿Òê"ޥȿá1ªlÞAGNbll3FGL J0521.7+0103NVSS J052140+010257?ïÿ¤'Ètú?O˜¥8=?ö
âÁ©!?O˜¥8÷?ïþr˜Ÿ?B_2¥¬5ý?'Öv²"?B_2¥¬5÷?ïõ"+Pt ?ZíÛÁ£I?T÷©_½´?ZíÛÁ£T?ïûì#•?4"õïø?@Oq«¿"?4"õï4FGL J0521.7+2112?Æw÷*Ë.À!iÓpóˆÀ6Þ¯\y}šÀ:­ò<ÈÞ+@]"ÿ‰b•?ýžøé‹Iu?'œÅ+	?§v™[ӇÉ@Çxþï^È@ȅ%ï'쿍4ö`€/¿ÙÇCáVF´¿ßûÛÙ>¿Û[$^.3š¿áø"ÁEZ'¿ÙÈý4s¥AGNbll3FGL J0521.7+2113TXS 0518+211?ïû1¹2?GY·ó*?CÃ;Å6¹?GY·ó?ïö›+?o
"K-Ji?RÉÉ©ÞÃÇ?o
"K-Je?ïyH,j?'~ÐE‹B?ÖÿÚr¿ß?'~ÐE‹@?ïÿ{ÕÎÊÆ?ÆÆj¤ ?…F&§Vß?ÆÆj£¸4FGL J0521.8-3848¿ÄqÞªíÎÀ@®1¤½º
À9ò÷Ãñ[øÀ<Yñ›@T¹³?ˆ@"C'OH=?·1NA+™a?©v(ù!?íºôB\›â@'̳¢Y\¿]kW´>W÷¿åÔ"°Õ¿ê1"ÝIó¿ä\¢b•÷N¿ätSŸx"¿ïü¿øÓçAGNbcu3FGL J0521.9-3847PKS 0520-388?ïþ¥N0Âð?"^Ág1?%«óÑô?"^Ág1Ž?ïþwrg"?A¬1¼.?(ˆÞI÷à?A¬1¼D?ïãQ`L?ouÔ ^Vk?l®îbŸ´³?ouÔ ^Vm?ïÿ'E+<Á?3X—pÁ?nµ0ω¡?3X—qÐ4FGL J0522.9-3628¿Ò›íþÛÀ@\] l‡À7Ÿmži3À;¦¾Ë'Iò@ðáºÅŽ@øÛÎÈO?"¸ý?¹Üä?³v¸îôiõ@ôAÿ~Ñ@U9˜R¿Ñèb8Yc¿â|Ê@€x¶¿ç°c	º"å¿çJ0i¿çäGbj-p¿át>KëAGNAGN3FGL J0522.9-3628PKS 0521-36?ïþ»¾hîW?!³ ¹CÊ?$Dq"â?!³ ¹Cº?ïøU·zf?f`OŠ[ñ¬?N©"g i?f`OŠ[ñ©?ïÀö°æ¡à?'´RFÁ=?"§Œ¯—?'´RFÁ8?ïþ¸ÿ¸Ñ?"ý™CG¶?$vðrҒ?"ý™CI&4FGL J0524.5+2839¿ÍÂ+MþqðÀ*Éòý¸þÀ9€ŽÌܽÀ;âF¼|ó@ X#8lÄ?þV>¶4ž?»àçáÑ?º ïZP?ÿ¨Ec·_}@ {KÆÓ?ì½q +Y¿â¾È'«hÏ¿ÛþcEÿڕVß	æ3¿ä;uÂ#ü_¿ØåÑëð~ƒAGNbcu3FGL J0524.4+2839NVSS J052429+283918?ïãVùTñ^?guVŒ1ä?l©«¡?guVŒ1Ý?ïÑÈ
cE?—³vw*?wÿúÎ\ä?—³vw)?ï'NÖ"?5?ˆY^äGQ?‹lJwp2—?ˆY^äGG?í¼¦—r!!?'Ã`+ƒØ?²ËDn÷?'Ã`+ƒÙ4FGL J0524.6-2819?à›þN冲À>c…@FA-À;"ƒ°jÀ<Ÿ˜!ÊU#@ˆâÖyt@®ˆ#Oa?ÛmN·ó÷´?̳ɛ"ñi?ðPêÄ.™@
'S6³ÆA?íJa¸¼-¿è3hb?_¿à5B!b¦=¿ë•›¨g'¶¿ïüËÝäw8?ïÈm54?AGNbcuPMN J0524-2818?ïþ*Z`Ç?1:ªCEú?-Z_™ób?1:ªCEø?ïþF¹'7?C*4?+"oFìx¬?C*4	?î〞‹a?"0… +?¡ÇöNyí?"0… *?ïþXM6t?? ½¶l«š0?*{,˜¼Ë? ½¶l«™è4FGL J0525.4-4600?éjT.J—ÃÀ@Öb=ú	À:bøwu'cÀ<dà?p@Ðÿ£ä¡*@'÷
èöÏ?Ãþuf^ƒÄ?©‰¼VÝÝ?ႣžU@#?ÿ·.Lïqè¿á÷ÀBû¨¿è¯•ÿÜſ㲁œøŸ¿à¡?«;®¿êp$ sRˆ¿åÛÍátϋAGNfsrq3FGL J0525.3-4558PKS 0524-460?ﯸÄ´¿?€³'ƒ‰Ù¿?"ÎÿRÐ?€³'ƒ‰ÙÀ?ïß`±+?ƒH?eó­?pOõý§j.?ƒH?eó­?ïe]ž­?ßsšáž|?"T^ŸŒ*€?ßsšáž{?ï¤?™˜Ü!?t¯í©Ù'?†ð™È÷j?t¯í©Ù*4FGL J0525.6-2008¿í¸Ì9`;À;ŒŸ±À:Ý
s†	šÀ<§Ç'#©R@ÚRý¨â¸?þÎE"I$?Î`ù•WÁ?ЬÞe%ž @vLe3`€@:@ºˆ'¿ïøªñ°²?ïöCže[O¿àdïY­¿ßÏËd—Ú'¿çf½+-«¿ïÿõEq#AGNbcu3FGL J0525.8-2014PMN J0525-2010?ï÷]óøðÎ?NµˆF>'?QDbK?NµˆF>'?ïãÌÐd?"ZH›ïgZ?l<sÿ/×?"ZH›ïgY?îº[†tbã?—¬",MäR?¤ZG˜¹ÑÐ?—¬",MäU?îødh†%Ã?µÀè?²? y¹w£¹?µÀè?²4FGL J0525.6-6013?Þµ†wÀ@ïz€Ïž8À9ۍs©ÏÀ<I<4c´Û@ £‹7?ûìUÿø?³Ãê%"N_?¥x¥X>°j?óo Ä0@?oߋì2?î*æþ§:l¿ä2ì@Ûgo¿ÞT"f¬‡¿ÐÍzÝð,¿â•†¢Z2¿¬éÏ£'7AGNbcu3FGL J0525.6-6013SUMSS J052542-601341?ïù¹†#«o?@cZÚH<?IçqRGú?@cZÚH<'?ïûÃãˆ%?^)ä¶ÍÖ?Cððqßhž?^)ä¶ÍÞ?ïçŠ
m—»?pvDÊþ?huõ'hE?pvDÊú?ï¾Ü1[g?i\¹/Þ¸?€zÈó©&t?i\¹/Þ¸4FGL J0525.8-0052¿ê'ÛÖ%þÀ3\‡D,»À9÷Í-DÜ©À<(Y‰QÞ@ÇRŠ¼\@C«Ë]a?À'Xßj3P?Ç¢C÷¦•+@܈皮m@
¯Ò"¢k?ïn¶—b&¿á×]Ÿmn¿ßr5§º¿ßO{hV+¿åýJä)िïñ£µ}AGNbllPMN J0525-0051?ïÎ×6;±?y0N(ïc{?xö"dâ'•?y0N(ïcz?ïòÈF(|?Tþ¢ûû?Zosݯ	q?Tþ¢ûý?î×ô@Ýù?›(€ý~?¢Ž€»ò o?›(€ý~?ïi⽊î?wžÿ2쁔?'èN¢=Ò?wžÿ2쁗4FGL J0526.1+6318¿áÖæ郋@.bTæâ!ÉÀ;"®"i›À=u‰ïØk@½"ªú¿ú?þ@ÊËjÍ?Ò¼)œ0¢µ?àÔ}e†l–@
dëVûX@q리§"¿ïÀ	ÿ÷?ïúDÕ&§¿Ì¹¯ä‰¬ç¿Ül±n¢u
¿ïÿ«±Ê?ïön¼v=tAGNbcu3FGL J0526.6+6321GB6 J0526+6317?ï¸|6iĆ?¦Vú©1?àòeŽÞo?¦Vú©1?#ëjR?®þâõ6q?‹\7%kº?®þâõ6p?éÎH7x½?µn×3BÈ?ÈÆߗ"?µn×3BÉ?ïðHRF?ŽdDNòD?öÿ•·:?ŽdDNòD4FGL J0526.2-4830¿ëk`¶öUÀ@à‰~™cÀ8QÔâEÀ;Œ½vîsç@ðmBùyÔ@Ï7ûïÐ? ¢òˆÉ×?±)¸
Hx@¾å@a @a v­†?°`Úá7'é¿àúõŸSí¾¿äv^½|¿ã–Ð[͆0¿ç»ÙÊâ¿ç^1¾éà.AGNfsrq3FGL J0526.2-4829PKS 0524-485?ïüÚà~QF?4%oɪÐ{?9(ü
uØ_?4%oɪД?ïûAzZ>»?`,IÊtß@?Bú—™?`,IÊtßA?ïՒÛCÆT?{2ßç"Ñ?u6'^Ö­?{2ßç"×?ïÿ©%&gº>ýT2¹Ñ-Ý?¶¶f ,>ýT2¹Ñ,ô4FGL J0526.3+2246?éJbCö†ÀÓÅyò4eÀ:bnŠ!WÀ<–C£Ã¿@!›i}r?ÿœ
Ý©"ã?Æ3–ÛNDÜ?°,¡r´?æ"ÿ[•R@$=Pš¿í®,Ε#é¿ì÷iCy¿ÔDhz<Ý¿à- Qn޿嚌Wè¿ÂèL:wJAGNbcu3FGL J0526.4+2247NVSS J052622+224801?ïÿ8ÌÊϖ?%œ9}A?æf¦
.ä?%œ9}$?ïÿ	®ƒHz?D•ŠCͪ?Ê/–ðßP?D•ŠCͪ0?ïò<¥˜•ï?g,\h–ßO?[†´ÎÔ >?g,\h–ß=?ï÷?U͘¤?Eäwàr7Â?QTdεr?Eäwàr7¾4FGL J0526.7-1519¿àâZ‡+=íÀ9~ÓØYÈÉÀ:d)uDÀ<FøE ›@Ý7•B?ýçOšr®?¾öڒ]:?ÁiíˆQ@ÅlC9@֌W¼ªk?ïÿÐ/WÜ`?Ö~?¶N[¿Øò°¡ôó¿àkÑtÒ9ô¿èŸÑâ5iÄ¿ÇE"/_iAGNbcuNVSS J052645-151900?ï<ƒo-?šÑuìÉò?˜oœr\Æ?šÑuìÉñ?ï&ß@Û?°¿kŒ<A>?›-äwäx?°¿kŒ<A>?í
˃œüó?¦ìÀÖØP?·©£ãb?¦ìÀÖØR?ì5ùÒ
=? ÷~÷|?¿¦P1o®? ÷~÷|4FGL J0527.3-6223?°ɟëÚ¤À@ÀœÜD9À;ÝùzªÁ	À<ý'œüûi@!ûÛ® ?ýç"Ä!?еâlvK?uÁ	þB?°ÌáßGgŒ?òBxåÄë¿ïþ×áÓÅ?ïÿJbú¡¿æk´ÿ{ µ¿Ô…4‡Ç	>¿äŸùš‹1!¿®$æ¿<@xAGNbcuPMN J0527-6225?ïÿ2LÜ×?~s‰û%?¼Vde<}?~s‰û}?ïÏV/Ó9¸?'žòçʛÜ?xTèc#?'žòçʛÜ?ïÜõŸ=E÷?xŕCŠ?q…0a]Å?xŕC‰ü?ï{8ˆŠ‡?¤Çdûˆ?Ÿøîî¯?¤Çdûˆ4FGL J0528.7-5920¿á¶5üƒ™õÀ@ĝàP7PÀ:~Æ/#ÚÀ<¢Û2Ál@|1~Ó?ÿþí+%Â?¿€®¼šq?­rp#ÃBy?ñ¨—³æKú@…žß(Äð¿êº ¸\R¿Á+m—C¿äOc 8o2¿Û¢"#揿×è÷»7ùì¿ëëgÝ^ëHAGNbll3FGL J0529.2-59171RXS J052846.9-592000?ïü§§	Ö?9êr7P?:ǺDZIa?9êr7?ïýŠEð¤?R÷wøïúÄ?3­Ðzß^´?R÷wøïúÌ?ïñˆ_Ž÷á?dœMíßAƒ?\ï@â@N?dœMíßA~?ïõ`¿=5d?CꢛœÅ?U>…•8°?CꢛœÐ4FGL J0529.1-0101¿ïûtzð4À2¸Å¸ÜUÀ:'ËÌòŒzÀ<#WóÝ@åü¤«Æm@'Èš8%
?Ýhüopü?Û*à~Zxò@0…ÔÀ·?ù|*­þ€y¿Ýpõ³ ?ïzËx8ö¿ç§¬_nû¿ë+$Á€hp¿Âðvà‡Û¿ï|þyØAGNbcuPMN J0529-0058?çْƒ]•M?Ë£Z
êè?ÐLÚùDÕg?Ë£Z
êè?æBvÍz9¢?Ó-KXÝ(E?Ó{eŒ½?Ó-KXÝ(E?åJÌ3_á?¸¶å/~wõ?ÕkØg™@>?¸¶å/~wõ?Ú.{°"ȳ?Äè9‰¦Ò?âèÂ'¶§?Äè9‰¦Ò4FGL J0529.1+0935?ïYÎÀ*Ú ¼8*À:&ä›ök,À<[}Ë@ C~Öʧ"@†‹ýϤ?¼x‹×åп…aC^EýÞ?Ëxëä•{@gmrU?á5žÎ^¿Ú>(¤äÑP¿èQxbè,¥¿á8Ï>ìúÀ¿Î/~Ȳ῿áå]‡š"•AGNbcu3FGL J0529.1+0933GB6 J0529+0934?ïõ¿IûÞ¼?Q/žRK|?TlB‰Ÿ?Q/žRKr?ïý"8Åvð?Pñþ(w?3f9ÔHu/?Pñþ(n?ïÒ¸ýÚA©?|͌zä?v£ß*ª?|͌zä¢?ïñ*ô"d?K÷k—x?]ª×6éý?K÷k—"4FGL J0529.3-7243?Þ'YKìxÀ?à.D¶é6À:YDéN
À<Q+"€ä@mÑ Ç
k@™µc#»Ç?À*ZÜð[r?±:ÂÇ;=?ñ4+
oÆ@4"Y8«m?ÛL»ð[¿×cL@Í¿èd^y]¿Ý"Âãü¿è˧¾uq¿äm´8PÍAGNbcu3FGL J0529.8-7242PKS 0530-727?ïøUþ`š?G­!ñûD?N¨}•?G­!ñûE?ïþžœDÕ«?C¾î*R/u?&;²¥FU?C¾î*R/\?ï¿nñ°Ÿ^?ƒbŒß½?€$C"Ø(d?ƒbŒß¿?ïý»žÎ§%?!ª©ñD´¹?2#	ŠÆÕ=?!ª©ñD´'4FGL J0529.4-0521?âÀ;v²LÀ4§"BAÃðÀ:	"V!uÀ;Údµ—&@'»Ÿ}ß)@E&z¾@?Èi
!A?Ñøá}³à@)=Ùb·@´Ž®¯?ÈqȨü¿ä®Á~ºñ¿ço£üÉë¿ë#3 hÖ-¿åù)Í¿ïîäŸQiAGNfsrqPMN J0529-0519?ìI€.×ü?·n$¿Ä?½³ÿæ‰@?·n$¿Ä?ë¹äp¤ŸÐ?Ŗaï¨O?Án=m€À?Ŗaï¨N?æèËçg>{?µÐNº¹?Ò.h11ƒ	?µÐNºº?黲?ðŒ?ªÛÞ­ÿã?É7=Î?ªÛÞ­ÿã4FGL J0530.9+1332¿îÊ`!0À&YWŠ*'À8Œ×òš½À;={á!îg@%C"d(I@­
?#?­êYXR…?ÑÅ9$ä»×@¤
COàé@0à?ÊN½þ'㟿Ûé
_¹ùá¿èVݲME¿é55¬E¿íàpÀ¿Ý,_#ÑìFAGNFSRQ3FGL J0530.8+1330PKS 0528+134?è[ò'¶?ÄùGID§[?Ïê7¥õ*?ÄùGID§[?ïåT	õ^?|oR QM‰?j«ö
è¢?|oR QM…?äš6÷Rrƒ?´ŒtfË?Ö˒[ú?´ŒtfÊ?ï.˜ 5–"?ŒZÃÀ¼kž?š,ëùM-C?ŒZÃÀ¼k4FGL J0532.0-4827¿ë)H3"k`À@fýüÁrÀ8;u!MÀ;g¤(hÔÖ@]
È°ÞZ@±ƒ›*"R?žTþ£Î?­?³è'¦
k>@c5X§a@ 
2~,€¼¿Ðëæ£7¨
¿Û@.Ä8©•¿âËcÁ'ý¿â[Kµà÷ý¿å6±'n"ÿê^òԞAGNBLL3FGL J0532.0-4827PMN J0531-4827?ïü¦Yù«î?5ÍÂ4"¿F?:Í02 ‰º?5ÍÂ4"¿U?ïú2¤$?`…a‰áΑ?G³7•ovâ?`…a‰áΘ?ï¯×ˆ:9?‡ßƒõ$+s?"
ûñqœ?‡ßƒõ$+z?ïÿõ1æ\í>ÒÆÐX£>՜3F(µO>ÒÆÐX¥4FGL J0532.6+0732¿ÞQ^Ê!ŽÀ+uîÇÉXÀ7"ñÓ'éÀ;B™Øƒº4@äÄ*;è¹@ž{€©ß?—w¾8Ɓ??¸
Xs‰@-š
^ÿ@kß/ûÆ5¿Âç<9¿áyÛX€Ê–¿åô>‹$¿äN'ÿú ÿéÂ}h‹…¿í*7/AGNFSRQ3FGL J0532.7+0732OG 050?ïæ ç°'?auWé]?i_Omù1?auWéc?ïâµ>£FÏ?€Úý%®?mJÁ\¹0?€Úý%®?ïÇփÅ?|"§¨
6ž?|ý"¾_?|"§¨
6—?ïÈÂKr?lò>(ÈA?{žÚrFýM?lò>(ÈD4FGL J0532.8-3941?îîþ<ãÀ?p‡¨ÖMÀ9¦Àð¸,À<]sWN›@¯B¼I@hÀ³¹Ö?°°"Üj ?¢ÊîË	K?ì•Õ>á<F@
£	Õk׿¿ß^TùM¿äÀVìÔª¿è¡Ü>ñ§¿èáyaë­c¿ßúþÄÄ
¿æïËoÌÂAGNbcu3FGL J0533.0-3939PKS 0531-397?ïÿG!nxK?énÛnáè?Ò0öŠ?énÛnâ3?ïþE£àá?Mó!îê?+¥Ïò	K?Mó!îêq?ïê'o"v?f\åa8?eùؐlŠÉ?f\åa8?ïý>OéÞå?)û/=.N*?6
€±ؤ?)û/=.Nm4FGL J0532.9-8325?ë"oI{ÔòÀ='xÝao‡À:ž‹¦'Ï¡À<Z›•\W@ ceù"ð@$á{°z‡?ĨèÁõÙ6?½š¸}ŠoZ?øNbS—@·ww°»Ÿ¿Ù‰§^(T]¿çv•žoû¿äêÖù¿ß ¾Q	¿ã~ÛþZ¿âÿ90£6AGNfsrq3FGL J0533.6-8323PKS 0541-834?ïÿ¡~ՃP?Κÿ?øN? JŸ,M?Κÿ?øÚ?ïþ­J‰…Î?<DªÛÑn?%+Wg£.6?<DªÛÑd?ïú£fð?^gI±m`?G©rg´;Ø?^gI±m`?ïÿZ"X9…?yñ⻋®?»´øÏ[€?yñ⻊4FGL J0533.0-8446¿Û'Ð,/ÉÍÀ<Ädf±åÁÀ;g
ÑZÀ<…ÚcŽDÒ@ùX¾2*J@œÈ='?É<;±î?­Ø°A ?Þb§Êà@ÅÌ8þ#\¿ÊEŸœh?À÷ö†¯‡¿ã{Âîýy=¿ègÍ<^¿ÒÞI¡ßŽE¿ïõ£ñpwAGNbcuPMN J0532-8447?ïýaÖI¨'?6ò¤¢¢|!?4ñM²»ÛÍ?6ò¤¢¢|V?ïþ®Ž˜6?B¯@_ÉÓ?%V|B?B¯@_ÉÔ?ïՄS{‹?u3a´1Æa?u=ÖB:u?u3a´1Æa?ïÿòóª?BLñ¾'"?ᡍêæ?BLñ¾'€4FGL J0533.1-6119?ï†<%I#ÖÀ@s(bõ˜žÀ:¨`"†ÉÀ<bûáN2@õÉe²@à´Zåÿ¤?Ì&ñ[wu?Çö?¨·o?ó	7KƧð?ïücÍÒ'Í¿ÕÙ6ýîü¿êBjۖ"¿ìÂ¥â'Qþ¿æ_Ë‹«D¿ïúè3Z `¿çb¿è¸¼AGNbcuMRC 0534-613A?ïóoQ¹¬å?q_@tˆö—?Y!\Œ¦1À?q_@tˆö•?ë5N´ —?ÎØ!›õ?ã*Å-}¥?ÎØ!›õ?ìØ ˆdˆ*?¦ÜÁÕ}·?¹>û¼Û¾®?¦ÜÁÕ}·?äËM.ÜÍ?ÀʛØö^?Öie¢Gæf?ÀʛØö^4FGL J0533.3-5549?ïÛzB²•"À@}Š2ôIÀ:')óÀ<rfàß©H@ý܌ˆd@£!ØG?вLBù¤Ç?ÕRåB˜?ÿ0ÈÚÏÄÏ@rßÆ?é¼|±¯¿æ_(뱔¿è'm{-ž¿ìâô÷ŽAw¿æ©Q2!»<¿ïÿ°NçÄ AGNbcuPMN J0533-5549?ïÜ?ùÂւ?|ÏæDÀ®ÿ?qà"¾¶?|ÏæDÀ¯?ïk
-{¢Ð?¡WWקe?'žZP‹¥÷?¡WWקe?ìã̖ÁSè?¦ÉÕs	÷'?¸á›Iõ`Ã?¦ÉÕs	÷'?î%[á%*v?—PmÏï?­ªAí­Xº?—PmÏï4FGL J0533.3+4823?×Vrš™¬@ {z_A®÷À8t7	‰À;ˆ"/•ð@ï-Ì­B@–n^'lV?T뱤í?¶./g5Ä@øDIÛì@Ðw€üj¿¢ÞAbd¾¿á›CRe'¢¿åÉ(½äQ¤¿å¿˜f"²Ð¿è§ÂòXw¿ëô—ìñ/ƒAGNfsrq3FGL J0533.2+4822TXS 0529+483?ïö)Ž¿D?Ke$²?S­ÔâwÙ?Ke$£?ïÞWš"X1?ˆ{Ø'"f?pÔ2îÓç€?ˆ{Ø'"f?ïÍ<)?{?Ýñ=‹z?ya÷kw|¼?{?Ýñ=‹|?ïÓú!+͙?`æ,rd¤b?vïj3­?`æ,rd¤a4FGL J0533.8-3749¿æo½û'À>ÜÊ>}QÀ:¬6ÉÀ¨ÒÀ<šq
"=@ba§ºÄ@m(<_+à?ÅôšÇ)?ÃCOàèã"?çÐ*_z@ ›'
`?ïôb¦h_¿èuüÜ_¿ßéÔ¯ð4¿ëƒB‹?å¿åÇ-†K<¿'üyº´¥AGNfsrq3FGL J0533.8-3754PKS 0532-378?ïõCFÕË?ˆˆ€ôHê?UÝyrThò?ˆˆ€ôHé?ïýï֊²?Q:"ªÎî?0‡)KªlÒ?Q:"ªÎó?9.Ì?‰5æ~[¯?‹±´LÙ?‰5æ~[«?ïû~;8Ä?0—ˆJ-p>?BÏô?0—ˆJ-pm4FGL J0536.0-2754?é£îC6HÀ;ÝCá`xÀ:ß9á£À<]HœQÿ@·FŽ"½"@Õ¶€Z-?Ëîc cbP?©sŠd§?ÖÏþ…Š@–ˆ¼|ž?î10Ÿ//ÿ箅^¤%9¿æÓZ»7y¿å·Š`@²x¿â¼(Fp'¿ïÿËA²Q÷AGNbcu3FGL J0535.6-2749PMN J0535-2751?ïþïGfI£? \œ·§'‡?!‰›eÄ? \œ·§'¬?ïýØ®
ÕÙ?Eª˜–ßÇ?1:©Q8
?Eª˜–ß»?ïÚ>dђ?uìùG;?ü?rþ`͗7D?uìùG;@?ïóEÁ8n?D…}ŠH¹ó?Yuü}$ë?D…}ŠH¹Ú4FGL J0536.2+1733?ïÞ´DbÌkÀ5çB™Ø"À:Fêóÿ@½À<eO1Ì@}4‰¢?þFÙóü¼?¢4GÛ5ñ?Οÿº4ï¡@ÃÔ»®—X@Jæº3Âû¿ïþR`Ÿýâ?ïýýu‹r¿ÏëŽÄS‡¿á9‹Â@Ð¿ä,õÌ W#¿ëþ? ÿ¿hAGNbllTXS 0533+175?ï¤*Í÷Ð?‹ŒÏÿ&¸K?†ÿ5L'?‹ŒÏÿ&¸J?ïœa«–"‡? Núh".?ˆç•ZÝÊ? Núh"/?ì°( %?«ççú¦?¿¢~ºÿ~Ü?«ççú¦?î%˜àÍ0?˜þf"+è?®m¦qó-?˜þf"+é4FGL J0536.4-3401?ïL›GWßÀ=}Š2ôIÀ8¡è
šó6À;Ý6'Ú9@©½H@û0<Þ­ ?¦'a;Ú È?µ'ƒ§"Ùì@í'ÞkZÂ@/cê¶Ó¿Ø6µž²Þ¿âÏi)Eƒ¿éY£àDxÖ¿æÖ_îÉ¿ïCB	[¿ïÿ²vìAGNfsrqPKS 0534-340?ïþã9?dpUm}?!Ìaör¿?dpUm|ý?ïüæK)>?T¦Œl?;xͦ¶
A?T¦Œ_?ï2'1½Œ?ˆÿ/îÓ?‹ó_sk?ˆÿ/îÓ?ïÿ}Ïê"?øÔ"ƒp?F½Íß?øÔ"ƒo14FGL J0536.4-3343?ëŒüÁ7[À=h"ƒ‡ß]À9L&ÉÀ;ÏÏò=@!‡	^Ú+?ú|Y¸:m?´âlFOD·?»rØ Ñ­m@
pÇZ@©U¯	¿ÙZÿ**¿¿è֞b+CP¿Ñ'd@ò8—¿ÛúcWh¿×?d"cýV¿Ð"c:AGNbll1RXS J053629.4-334302?ïþ'ê6à?(—-¥`¾?-\'ÿc?(—-¥a?ïõ©Ës=O?uË«ÃÎ?T¬i…aµ?uË«ÃÎ?ïÚ®8Ž¨?xw2ë`Ø?r¨ã¸«ýß?xw2ë`Ý?rQ¢?~t)¡hñ?Š\£k 8?~t)¡hî4FGL J0536.5-2548¿îØiqÀ;Á?ÐÐhÀ:òÚ¬‰`fÀ<¦"Òb8@ 8»*
Ä?ûî[ãU¥N?Ç.DáÜS?Ãí†*Ñæ?üÉåvç½ê?üku.€F¿ìðdaS'?ïâèÍ´SY?É.Êî¦;i¿â5Z 	 =¿ÛrMºÈé=¿ÝïN¢$'–AGNbcuGALEXASC J053626.90-254747.9?ïõ‰•È?Uk*8»}?UâìÔou?Uk*8»‡?ïñ4eç?€\Ä5I,K?]—Ñã44ê?€\Ä5I,J?ïºh2ø=?|(C¥³Ñ?eóAðœí?|(C¥³Ñ?ï&¼™BY ?†Dçfœx-?›(l×´Ûö?†Dçfœx/4FGL J0537.7-5717¿µ½5þ•¯6À@2'!%¶À:/Pž~éÀ<}`Z³«@ñ:ǧ?ý~"_¦XÅ?ÁÁ¹my?ÆBº$Sœ_@w´_½Œ@j/š¢X/?ïÉ­}ÒÝ¿æÙäãD¿Õë&>®Ÿ¿ÜèÿI Û¿ãèZ&½+¿æDiò!vAGNbll3FGL J0537.4-57171RXS J053749.3-571844?ïÉðP]š¤?{àV]SOá?{×Ñ2®m?{àV]SOß?ïï´ëË`ø?wsŠý)£?`K4Ÿ(?wsŠý)£?ï@ Æ£7?'&vO3"?—ûç+žù2?'&vO3 ?ïÒßÍÒ­?€¾¨íË»_?¥¤Eªt?€¾¨íË»^4FGL J0538.2-3910?êN€e2–À>LøŠ/À:îäŸQiÀ<­C³³÷@ ͪÃ7£?þS#ä
Öô?ÄUaÆÄu?±ÞfRDp?îªõÂ9uí@}
yæ ¿î˜×'2tÇ?ïömzVÞ3¿Ø70£‹àÉ¿Ý;êý9|#¿ã2½ÂmοÜl+Â{AGNbll3FGL J0538.4-3909NVSS J053810-390844?ïÿžÓƒ9?õrg®³†?K>òÆ?õrg®´b?ïþLA5"ì?GKÂ7ÌPÁ?+;짱M?GKÂ7ÌPÊ?ïôÙÕ3²¦?_›_Ÿ.QJ?VLU˜š²­?_›_Ÿ.Qo?ïýYÊU?*…¿	¤ð?51¯ÕX
?*…¿	¤ï¤4FGL J0538.6+0443?âì^ŸÚ´$À+³ý">5ÆÀ;]{ÜqÀ<g$€	@!Ã%	òó?ò«^Öw?âvÞñ'?ãÓÓÃt^@ÆQÒZ«@"6ÙÁ¿îè"1 ‹ü¿âݜ'éS¿ä5åàD"ð?â¼(+ì¿ØÖ'\ä¿àJÂ7óaAGNbcuNVSS J053847+044222?ïãÐ9þ?héh<f¡Ø?l/áâÆÇ?héh<f¡Û?ïüJsP­?V¶ìø6?=¬eâ—?V¶ìø0?ïs,8›k?ŒÛÆϘ?'šxüŒ'±?ŒÛÆÏŸ?ïé(ÇÔ<?aâÕÇt?f×8+Ãìú?aâÕÇu4FGL J0538.8-4405?Ԇ—N)ÅÀ?"á¬WâÀ6…C>C1®À:áUÁÓt‡@¹&>{@%ن³U?…/‹]ìšH?¯¿!M@$qJG
@"_ða俚£xHCÄ.¿ÝUý£z´¿âŠ¨ÀSÓ¿ás¤r:¯ÿ¿å~bÁ–7å¿æHdÞ&‹AGNBLL3FGL J0538.8-4405PKS 0537-441?ïñy»‰eû?XÀï7Tۊ?]ˆí4
D?XÀï7TÛ{?ïå[¹Êj[?‡ri?%?j¤F5•¦!?‡ri?&?ï¯Å€°°?ˆæ­žüi±?"ŸÓþÁ?ˆæ­žüi²?ïÿfX÷u¥?8±Ò
÷N?4áK2	?8±Ò
÷a4FGL J0539.0+1644?ÛZ­Ú+w<À²ðZpŽÞÀ:?LÔÄèÓÀ<ƒræ§i@ À-+1\?üF€'q^è?ÇÄÚº÷f?Ð#nå;µ@`q$/Š1@Rëä?/@¿ïÿüñý?ïý~›;…¿ÜkÊSuÈÚ¿Å÷÷ÛÉ¿áL«tp–¿ìÓ51:4¯AGNbcu3FGL J0538.9+1646NVSS J053855+164612?ïô
`Š<J?W$¶RÛ>è?Wå>ë‡l#?W$¶RÛ>ä?ïöYÌÜ]$?~†œ³WôW?SLfGE¸‰?~†œ³WôY?î4³Ã´üe? @û³§ã?¬´ÃÄ°9©? @û³§ä?ïŒ	ÑßHL?{VýÌZ?Œý‹ˆ-ìù?{VýÌZ4FGL J0539.6+1432¿ïûô‡ž¯À!_ôºQ À93Ô¶¦ÛÀ;©žÙt{@ó+kh®À@}/Bãª_?¹LFT£w?Ågù¹iï@§î%âè˜@çZ™B?ïø¬N¨À¿Ýã܉Ù2¿ç1Ubˆ
{¿æ'òÁS¿î™i}Èâ¿á€‡—ůAGNFSRQ3FGL J0539.8+1434TXS 0536+145?ï狝`Æ?g˜1iµ?htbŸ<z-?g˜1i¶?ïüˆUáÉ?TñãM$ƒ?;½Pó´\?TñãM$"?íÓXdoœ:?¡
VºnL?±e<܃;?¡
VºnL?ïúJ"W÷?8̸ÙóŠ?F×v #ƒ?8̸ÙóŠ94FGL J0539.7-0521c¿á÷œ¶3ÔëÀ2_5ŸôýmÀ9ə~Á¦ÿÀ;T²ò03¤@¶FÉ)@0Þ@'—?ÑáõRýÔ?äŽàØóL@-d"¿G©?û½DC¦É¿â†¤^ïy ¿ÑYƒÿÔa¿çãW=SŒ¿îýÄupÅ¿ïþï~þbÇ?ïýß(ïãRAGNbcu3FGL J0539.2-0536TXS 0537-0524?Þ¶#äúŒ£?Ò@œóLPZ?à¤î
'¹¯?Ò@œóLPZ?Ê¡¥N_E?Ñ
1šj?éW–»¬h.?Ñ
1šj?Ô5f¢µ ?¸À	ԀÅ|?ååLÿ®¥p?¸À	ԀÅ|?"|k–»u?†œJäX×å?ïd£O%?†œJäX×å4FGL J0539.9-2839?쫦ߍÀ;FE^®âÀ8ÜhìR¤À<:kHM@æo¨"µ@jnü7£?¤àš_]u?¼£çü(/@IŽ|/%‡@³puÞÔa¿ÒԽ렿æV¡ÍD¿é®/RÓâk¿êýDcÝ*¿éÒ%Âu:¿ïÿùëñAGNfsrq3FGL J0540.0-2837PKS 0537-286?ïÿiâÚ»d?P|j oÒ?䨓oJ?P|j q½?ï÷mQMŽ?hùÚÖ?1?På%]dâŠ?hùÚÖ?3?­[Ç?‡C¶h	û?ŠÞ"©:Ne?‡C¶h	ÿ?ïßig6
/?`ÑPo?pKLdúèc?`ÑPn4FGL J0540.0+1209?àã'TFkÀ#©QçS`ÐÀ:MY0ó½ÒÀ<ږ¹ëI@1tÅyÇA@b‹°¢Ê›?ÁÅ«âqz?¦í´£á8?ç*êßÝJÉ?ÿêEko׿ß;ž¼™#¿àÇ÷°¦%™¿è""j«o…¿åÂù¿ŸԿՏF¹!õ¿ì©«àn[AGNbcu3FGL J0540.0+1208NVSS J054005+120955?ïÓº3rë?käÀþÔØ|?v"æF¿
1?käÀþÔØv?ïõ'u偳?pSMÏ÷ûl?Tû4üš?pSMÏ÷ûj?ïgh%	º¬?Œs"8Òs?"û^Ȫu?Œs"8Òs?ï§Ñ÷ß2?t"˜Þ?†'3zl?t"˜Þ4FGL J0540.5+5823¿ïÿ䞬>ñ@,‡îõìÀ9·É°¸šÀ<1µ°P•D@ {Md·»?ÿ4ùÜÐP?° ÄÍ¿ƒäª
I…?×^ëîù@ê6êø²?ïªÏL¿µTÂ$'Q©¿æyWÊÆb¿Öt{/PP¿â*@Õ³P¿Á6"f\UkAGNbll3FGL J0540.4+5823GB6 J0540+5823?ïù©í!H?AŸÙ.P%^?IXI¿zã*?AŸÙ.P%]?ïù`‡:bä?k•ã??J}ãti}?k•ã?
?ïçRꨙ?pòÒ×½ú-?h­€Wf·?pòÒ×½ú,?ïÏ@,]<ï?fB߀çÛ?x_éÑaˆò?fB߀çá4FGL J0540.8-5415¿ÕZ£s`À?ڄœ²RÎÀ9Ö­'¿À<0'5G	ª@P®äY†Y@×¢~D©}?·…ß'˜J?¶vÙ{0øÆ?ù¸ÞÙ>Ë@üwÒÊgÃ?éÕá[Ð
¿àÚçœr<¿éW°´hR¿é
Öøj
¿é–š«èP·¿Ó3«¾Š>ÞAGNfsrq3FGL J0540.5-5416PKS 0539-543?ïüïÕ¯4?78ˆáJ_?8R‡d‰?78ˆáJ^ý?ïþª¥3ÚÉ?@Ü>¯¨7æ?%U¬ÂSqê?@Ü>¯¨7è?ï²,M
?'¹Cú݃q?ƒtì¼»zà?'¹Cú݃p?ïþY•E3?^Î2Ålþ?*f«¬ÎµÝ?^Î2Åmg4FGL J0541.1-4854¿Ó1Ō$ÇÀ?[ÂôÀ;Jh˜À<»ú`ƒÎV@ I'ˆ°é?þláłU°?ʧ6eAÎ?±ç0Ñ.0j?æ£ø'Ä@Áp¾0a?ïà¿ÞQÚh¿ã8 7­ì7¿×@-…öú¿æûm"X9? ýÜåÑw¿éÝ}‰˜š–AGNbcu1RXS J054106.1-485408?ïÿU5̛ë?œÏЍO"?YFl''¼?œÏЍO)?ïþ³éÓà?Añç†ú:?$Ábϒ?Añç†ú7?ïã}2U–?sâ¡?s|V?l'ͪiâØ?sâ¡?s|L?ïü,{å?2±VM¥ì)??îœ' Ò?2±VM¥ì:4FGL J0541.4-7334¿Ó‡±3HGÀ>Þy!°À:Îނö À<qÏI~Ï@D>·Ë³È@o?¾[ðÂ?ÇÍ|µˆ7œ?´e8>ŠÕ?ìÌxžÍ5'@¹\Øs?îñÓ'é|¿æPµà!=g¿åt!N¿ã%€Uпæ¢'Õ¿ï÷z?·%AGNbcuPKS 0542-735?ï÷7÷–ñ?KbÓ8ö'?Q'úÒ Q?KbÓ8ö¡?ïùKêÓG•?e¿UqWrX?JÐT²á®`?e¿UqWr[?ï×¹'×Ý?sÏÞ`¦Ø?tr£7Ô?sÏÞ`¦Ø?ï¼JPe?fÀ‹U(»è?€íxkþfá?fÀ‹U(»é4FGL J0541.6-0541¿íÍ RdÀ2üÞãOÆÀ9®Äjþ{œÀ;]±÷^pÏ@,¤ÅFƎ@ÙEnŸ?ȪÚ3½œ®?Æ6·L2º@	zÓõ@S¬–¡l¢?ïþVèD!˜¿à.ñàW™¿è:#aÔÜ¿êsp-…¿ïçæcvÇÝ¿íyº×AGNfsrq1FGL J0540.9-0547PKS 0539-057?ï7œºŽ?¡<§Ìê©?™Œh½®H?¡<§Ìê©?ç	ȗÎõV?Ñæ¦OÊÆi?ÑìnÐbV?Ñæ¦OÊÆi?ꥇ,Tɯ?²B,ÓÙÒ.?ÅiãN¬ÙB?²B,ÓÙÒ.?â²çÝKž?·§ÚklBÀ?ښ1îEhÅ?·§ÚklBÀ4FGL J0542.4+3547c¿àµx¯·@ÔÏr™À9{ÿL{ٕÀ;/(«ôž@ý~®Ü¡×@cwá¸í?É©½(?^?lj£Aãû@gÀôQv?ø?	ˆ??ïÿÝ/ñ_S¿½èplN²Á¿é}ž¼C¿çQ˜Wz:¿èªŒ€¬bÊ¿ïý¸È3
AGNbcuNVSS J054218+3541490?äU"Zq?ÏängÍþ?×TÙKÿö?ÏängÍý?ÔEÃÔf	j?ÒY:d×µ;?åÝÌûK?ÒY:d×µ;?â£Ò‹¤é?¼æ`g{<?Ú¸Zè·À0?¼æ`g{<?Ó.FÒñ?±'Þq"¦?æwhÜö‡?±'Þq"¦4FGL J0542.8-3458?Ôâäà¡ÍDÀ<u?|ÌÀ;§W>«6zÀ<åÄ÷u³@ Ó,nÈà"?ý<ÙTšŒ?Ѷb'œOV?¶wÁ­‰æs?ènò&"©x?÷p'¢Ü8{?àÈ'Kžd¿ãÏi_?*¸¿·ýÌ^'Ýh¿àG>îRX'¿ÔÎÄɞ¿Ü œ'­ýAGNbcuPMN J0542-3500?ïþ¹õS?+ï¤ÌóM?.4`ªÎºW?+ï¤Ìó0?ïöøëó1?p*9jd
?R)üž!?p*9jd	?ïéÝTDñ?qzDŠ"×ü?f"î«»9?qzDŠ"Ø?ïÃ-ÄÐÛ¿?j=gŠAÅý?~i—' c?j=gŠAÅû4FGL J0542.9-0913?ïäèuæ)nÀ3^rÚ/­À8Óp]`-gÀ;*[rÏ*@¸	FOÆ@×üMÃØ?´ìÈÀ£ž«?ÄyÔttF@¥!Whœ¢@ãðŠD?îÛD)$¼¿Üø,AQ"¿é¡Þ¹q¦¿æ# ÄS¿êÚ÷½'E¿ï´~!nÑAGNbcu3FGL J0542.5-0907cPMN J0542-0913?ïÈø^1T?|zŠ¶
S£?{ƒÐç}Ö(?|zŠ¶
S¦?ì^:cÂB?ÊÁ†4
"a?½6,áíö?ÊÁ†4
"a?ë¼4"Ó?­ábB9Y?Ãù/t¯?­ábB9X?ìÄn®•? 1,õ©Ão?¹ÜŠ¿ÓT? 1,õ©Ão4FGL J0543.9-5531?í°ø;%VÀ?z]9–úƒÀ8´ŸVqüÀ; L?b@êˆü¾W?ú'åÂg=?¦ –R?±Íߢú@ìÿdύq@)øH¦Œò?ïÍϖ«¨¿¿Í­$Ù¿ÙW97Y2¡¿Ôh>Ã4G°¿Ûï?='—t¿Ùâöúó¦«AGNbll3FGL J0543.9-55311RXS J054357.3-553206?ïþ¡-t8ý?$(IwÌ5c?%í(¼p,`?$(IwÌ5'?ïø¶VÛíh?d){û!AÁ?M&¤JX¢?d){û!AÇ?ïܞ¼Ž'
?uûEÁJæ?q°¡¸·yh?uûEÁJç?ïç'!o?UÁÏ2_?hnäåސ}?UÁÏ2a4FGL J0545.0+0613c?¸âî됍.À'qýiôÀ9ì0Ûj'À;¡[wN@ź+µe@ñèæ?ÎUlƒ‹æ(?âÕýÞâ@†I%ÿÃ@³ƒJLÕF?çÕ7Ÿ©~¿Êø›‡°c¿ê¤0ÌP¦¿ð?ð¿æbb™RLAGNbcuNVSS J054529+061955 ?æg[¦åü?Ëþ(ü•?Ó1ñH²4
?Ëþ(ü•?ì,
4¾?ËoŸuoE?¾Ÿ®_Çj	?ËoŸuoE?àé~DÅØ?¼÷÷Žƒ«?Þ-ÿvtM?¼÷÷Žƒ¬?íð­c•Xƒ?¯Dñî<¼œ?°z"ãU;é?¯Dñî<¼œ4FGL J0546.9-2206?ìg"ªÐÚÀ7 E®_úÀ;~?SÒåìÀ<̍‰Àß@!
¯Û¥W¾?ý¥È–Ý&·?˸é?©"ô›ó»ú?⥡õ¿?ÿëWã俗…"úÙ®?ïùõß덂¿ç¿Àéz-¿Ö—
]¦ú*¿ã/5b7'£¿½ÿ¹3<îHAGNbll1RXS J054656.9-220500?ïý±¶±Ø?1ŠsJj?2rOÒq='?1ŠsJiý?ïõ»"ÿð?vq¥Žp
µ?TˆÖÐÐ?vq¥Žp
¶?ïï	xxÑc?a‰*¦?`ö‡‡.›Î?a‰*¦?ïɅ¢&?loC]
L?{=.ð}lé?loC]
K4FGL J0548.5-5218¿ãZéãQÀ>‹¨çv°À;dÿÑÜ×À<àNú9¢@63Ÿi½3?þ^Õ®Þ]?ÓDE>Îqè?Ý\Šû>Ë@ØÌ<"Í@à\Õîßq¿ïÿ¾…{ª?ïâFj^?Çi^GG¿á'V½•!¿ë•ö¬š'^¿ïíFõ‡ÖùAGNbcuPMN J0548-5218?ïß͝¿U?r•ˆ©ÿ.?p1 pT©?r•ˆ©ÿ.?ïîâƒ8NW?z*òY:ž?a|DZ¨¤?z*òY:™?íXÃ¥¼×?¡©Ö)‰Ñb?µ9âÒG'?¡©Ö)‰Ñb?îÚԎÏ_Õ?¯[Ú-è~?¢R·
ž?¯[Ú-è~4FGL J0549.0+3258c?á7Ý.Ā@Ä{'W]µÀ:e²ÑyøÀ<Ô€ö@ ύ3YÉ ?ÿ­*:f-\?ĚS¾C4?²þ½à ¿(?ïïãB/$†@‹99\˜?ìÏt…
?í÷y´!]?¨]‰a×Ð%¿ãµÁM<ɵ¿ßЍ]b²¿Þ•Á}ŽK2AGNbcuGB6 J0549+3258 ?ïÙi'°—°?t;[a"vÆ?sK>§´'¾?t;[a"vÁ?ïÞ¦ÙÃÕ?Žƒ)ó¿@¥?p¬"r'?Žƒ)ó¿@¤?ï£5è"?†Y~™ü-Ž?‡2…à>Ÿ?†Y~™ü-'?ïÛB+éÛ?1qÛøa?Ÿd—º'Ä¿?1qÛøb4FGL J0550.3-5733¿ÜV 5
6À>´üvÄÀ;‡‹z&À<§—…Ã#@@§c±«3@¸¤ÁëÈ;?Â{A–£E?}s±¸ç?»i"d O@3Yàqs?ï½|˜%¿Ý¤q"&À´¿ç>A¹Þ³¿äz/ ~û‰¿êBª¿±±=?ÛÒHÂf—dAGNfsrqPKS 0549-575?ïóSY«Íª?Zb&—"?YYL¨d©P?Zb&—‡?ïþ©ßmT*?=A*»ú ?%b	*½k¨?=A*»úí?ﺽ²ÓÆh?'_vJÒ?P"KeØ?'_vJÎ?ïùkC•hˆ?9Ÿöß&È×?JRñª]àà?9Ÿöß&ÈÊ4FGL J0550.5-3216?ל´fè´À:.—á2µ_À:EÂHåL À<eg?ª9û@ 2x'$"?þÔóý">6?¶™÷']ῚÎL‡JÀ ?äØ<l—ØÏ@–ß~*R¿ÁaL ?¿â™baÉô€¿ãžë}'ü¿ÃøÄwhÂ6¿åø£_–¦¿È¢›[e¬AGNbll3FGL J0550.6-3217PKS 0548-322?ïú9
?@C,[.×?GïÕËÅ7?@C,[.ä?ïý ‡JU?RÀ™ú—ýI?7nûÅ­X?RÀ™ú—ýF?ïò×W'ò?a¾L«ô s?ZQPÝþ?a¾L«ô }?ïàR—Ù?\TÄê!i?o­þðh$Ú?\TÄê!i4FGL J0550.9+2552c?àZbœó¿â"Ùîô?À9æã3@Ÿ-À;\€¸!D@q`-…Ÿ?þ£Ah€?ÔVK¼J?ä±il«$@'Á¯bY?÷îÿ&¼,¿ítD
õ?í®¡žJÙB¿ÞГ@d8¿äì;\Í`q¿ïüá1ޟ]?ïzô}jäÐAGNbcuNVSS J055119+254909(?߉Ù>m?Ï÷¤{ã?à;~}`Ê?Ï÷¤{ã?Üg@,Â8]?טn˜Îð?áÌ_éžãÒ?טn˜Îð?ڑڶ¼¾÷?¶HŸ#Ý?â·¤¡ "?¶HŸ#Ý?ÑI*x^mï?º
Žqî¯?ç[jÃÐÉ	?º
Žqî¯4FGL J0551.0-1622?Á½ÊƒÀ4ŽùÛ"ÐåÀ;jNÕP)
À=<±¥)@z8MNgl@‰üpy?Ôa):¶à&?ïü辚Úâ@n'"šV@Ÿêw­‹"¿ïè—8å?ïý2%9þ¿«s€]æï¿æIàô¡þ¿ì³·RDÌ¿ïÿæÀ
AGNbcuPMN J0550-1621?êUÕâ¤ß´?ÆÒºû»ÄR?ƨ¨ul3?ÆÒºû»ÄR?ë×é왏ç?ÍÛÜ#"?À XM™Àh?ÍÛÜ#"?ݲÎL@՜?¸ÊØä-£?á&˜Ùߕ2?¸ÊØä-£?ç_L—wє?¶œpè×÷_?ÑAfÑ\Ù?¶œpè×÷_4FGL J0551.8-3517¿à~kË"CÀ:¿ÿ›V2<À;_ø[ÆÐÀ<®}1"Š@7ÐVD/Z@80êÄ?Éãã¿­€¿ªÕ!ș?àèøFΫ@û‰"Óê¿ÐÊaÛ<Q¿èsáÿcøο蘰C)J¿Ò·ÇíiûF¿áß& {±¿ïÿž´JAGNbcuPMN J0551-3515?ïü}ú
??2½cÒÀzï?</w–?2½cÒÀ{.?ïý¤—Dͯ?W9Q5Xð?2ÛEْ†?W9Q5Xä?ï҄œQl¡?u{¿	-?v½±×I¯
?u{¿	-?ïú\Ë	Œ?8Õ=à3?GæŒÓÙÏæ?8Õ=ßí4FGL J0552.4+3755¿ïHsòI@G¹EÅÀ9£4EHßÀ;º]éÀ"š@n¬`@¡59°€?Á—O Ò?Á2ZR½?üzžF§">?ÿÿa¨â¿Ðqm*¥Æ¿à)û|ÀÙ¿è¤@¼ˆ±ë¿åPŸ?J螱Áƒ˜{¿çWÿñ<nAGNbcuB3 0548+378B?år—Ӑ¿?ȃ¹¡žU?ÕÐXށÌ?ȃ¹¡žU?é¸êo=öw?ʔPC¬¯œ?ÉVC&$?ʔPC¬¯?éLª›¼¥?¶-¢õî.x?ÊÍU'
m?¶-¢õî.x?êÎc1×ã?¨ÉržÏ?ÄÆs;¼ s?¨ÉržÎ4FGL J0552.8+0313¿áÖÈõöùaÀ&ñÖ1riÀ9Øe8hýÀ;eQ‡²‰@q¡L–[¢@Fü"û­‹?Ç´°¶Áš?ÑàZ]āO@
ûÅ<@ÿ7VÙUœ¿×í\¤Æž_¿ß&H>2?ÿäÛâ…ï¿èòÁˆËëü¿å«hÎör¹¿ïþ3AGNbcuPKS 0550+032?ï¤6y?œ[Zhc_?žëY1?œ[Zhc_?ïíÄþ¿q<?†*¼Áu›?b;@ŽÂI?†*¼Áu?ém3¾UÐ?®í̾Eñ?ÊK1«ð¾?®í̾Eð?ï6üNBfI?‰S1Ô*?™ v7³6á?‰S1Ô)4FGL J0553.5-2034?ìÍ¿ªmâ3À5ž YžØÀ9Ýu&Ê;À<­ê‰v6@~¸w«?ü9 4¾M®?·
´ÉuÕ?Ã׎\Nµp@ÿW}•@¼E˜•?ïüÀO(\¿Úx6<Òï&¿Ñ°'#Ùy¿ÝóÎCoks¿áè–!?é¿å[Û]‰HAGNbll3FGL J0553.5-2036NVSS J055333-203417?ïɧõ¡Ã?V¦'H,?{q¬/¸?V¦'H,?ï¢p‹½[V?¥¾#ãÔÍ?‡cÝ©*o?¥¾#ãÔÏ?î綉d?šøON?¡"ž—iÄ?šøON?î÷Ìr»ž?…WEsÔC? ƒ8ÔN6,?…WEsÔC4FGL J0554.3-1009c¿ß!q+ÖÀ1<yÄ<hÀ9ÖÁ['—À;¢˜¢ô@>ñŒõœ@W'"¬Ó2?Ì°rùòŸÅ?Òc¿m@ë_ïIÏ@☡!"e?ïû%|'¿ÞôÔRÓ«¿ç¸}õÏ$–¿í—'"Yœ)¿âùƒ¿g´o¿ïü`8NûçAGNbcuPMN J0555-1002!?î.a'úߖ?°‰ëÕdfé?­çÐR"?°‰ëÕdfé?ìýÿ2PB2?®Þ€µ´?¸m}îw?®Þ€µ´?å@­—¥ãú?¶M'_àI'?Õ~¤Ð´8
?¶M'_àI?ì%"(š N?¦9Ú|"¨?¾Ó^»*ý†?¦9Ú|"§4FGL J0555.1+0304¿ë
ÇǧMøÀ&¬ÿ§ëlÀ9•'ußÀ;;\ºëù¹@"©	#?J@X$¹ó¬5?ÒXDЩ*?݀£(Ž"ƒ@kE®_ú<@Üƒ#5?ï½<Á§TÿÆ?¹éÆ,Ë¿êz73rô¿êm3t¡'Œ¿êõÀv}4ß¿Ò¶žb+CPAGNbcuGB6 J0555+0304?ïõÀZ¬?˜ þZe•¼?‹Âéz?˜ þZe•¼?æn'Þ²co?ҟgø´Â®?Ó#°B›9"?ҟgø´Â®?ç'Wº¾è?³ãNd?ÑɱPŠ'0?³ãNd?áß½J´ÆÕ?»j7r‹v?Ü@…j–rV?»j7r‹v4FGL J0555.6+3947¿Ü†^ë-Ã@&7yéÐêÀ8ÃÑv¹À;™Ø)!az@—v³·X@-µ@å£?¯ó–Kwx?Êe*&D7g@Á+àŠð@$5f¿&Ç¿ÛMÓÈi½¿ã½R ^DY¿ê¨ðN²¿ë-€@Ø¿î9Ìzd¿ïÿþó…õAGNfsrqB2 0552+39A?ïÌÁ|ùë?~Áà½,?yŸAƒ
uo?~Áà½/?ïÓ´¹7ZÇ?"oò-6Á?v%£dR›É?"oò-6Â?íP|Քæ?¤³á ;#\?µ|Ó{XÇ?¤³á ;#\?ïþ×Gä|?wü›©<çj?‹ÀJ.à¬?wü›©<çj4FGL J0556.2-4352?åƒPà\þ(À;ö:\`‰À:&þìɹÀ<G|¾—ä@Á8jª™?ýª½þÓ°?¹œµØ¿tJ?ÄZã»Ñ§Ó@	®¢?Zˆã@	茿ð?ð¿ÑÄLá<P¿áânÁŒ¿ã©LŒ ¿è"¤o¶AGNbll3FGL J0556.0-4353SUMSS J055618-435146?ïüdTλ?6'¢«µ$^?<Ý_ùŠ*Ú?6'¢«µ$w?ïø0}ºXÛ?udÖ:6ݯ?O>	œ'ñ?udÖ:6Ý«?ï€üqñT?‰®tÇ"ß?À・ë]?‰®tÇ"Ý?ïß|íP'	?apÄ(Ö¤?pA‰W¾û¼?apÄ(֟4FGL J0557.3-0615?Öу.õcÀ-ºIÂÁ±À:''¡WÓüÀ<*ý"û|ä@!7œÏY?ÿ—{ž?ÂàU*S懿t¼™4*:L?©¦^ÄԎ?ÿPûB÷?Þ­¥,tÓ¿«ƒÕü»Ú¿èí±´B'L¿Öð½!´Õ¿á,ï¢9Ñ2?²¼ŽŽ#AGNbcu1RXS J055717.0-061705?ïó—"-ÍÆ?Uå9íÁ:Ð?XÑ»¤dr?Uå9íÁ:Û?ïù"²Oñ?fOÚÀM¶?K—u6À=^?fOÚÀM±?ïÜÊ"D?sXú-?qšùµÝ±º?sXú,û?ï¿ãã5?kUû£Oï‰?€9¼G2å?kUû£Oïˆ4FGL J0557.6-0721?ï¦K]âÀ. ù	kºÀ:ÔdÓ¿/UÀ<@Ñ0ߛÜ@!GÝcp?ÿ¢ºtÛt/?Èêo_‰Rz?Ê¥Þ©÷"?ÉU·­¢@ÂÌå¤?î¥ÉB©É¿Æ3IÃîVà¿ì"֎ín-?¦ùQÁ¿ßË¿ñò÷¿Í9б3AGNbcu3FGL J0557.7-0720PMN J0557-0719?ïÿ[÷<Ǘ?ø°<dÒþ?g
'Ì?ø°<dӖ?ïþÈà<B?@)Êȱõw?#qÿŒ<k?@)Êȱõ'?ïè]ÎA%?s`Dº–?gé¢1¾ÛÌ?s`Dº™?ïûjãàø¾?4ö…ºl?BTp|¥?4ö…º4FGL J0558.0-3837?ïf™U&úCÀ:mYėtÀ9¢&¶ÁÉÀ<.‡'§
ö@ʹø´²$?ýnz[æ±?³Ò<^'A?¬Ü	֘}?ù&رÝ]@4hwä?íCy1DEª¿â$;H«j|¿Ü»µƒ+ß¿ÛÕгÚ
¿Ú/¡ãêöƒ¿â¤®ÀÈ1²AGNbll3FGL J0558.1-3838EXO 0556.4-3838?ïúÂ\)…p?F
†ñ‡0?DöYêF?F
†ñ‡,?ïû›ˆÞk
?YZò6øÃ?A'܆SÊ­?YZò6øÏ?ïíÛ0-w ?jYð-½?b$Ï҈ÞX?jYð-É?ïÀÿ€?hÂÏ'Û?ñ€sÀƒ?hÂÏ'Ü4FGL J0558.1-2859¿âŒ}¿Í±À7™0ߛÜjÀ:Ñ]ÓÀ<šz¦]Í@Œ›Ág
@æÜB‹–?˒ºNðÔ?Æp˄£=\?ø™åi{Ĝ@Ç9©Ml?ïü›ÇqC9¿ã¥ÞPݾ¿æ4Š¡.8x¿åÖÇAÈwS¿ïüõ$®5¿ïف±E‡ÊAGNbcuTXS 0556-289?ïñ
¡p­E?hçVKp?]ä½¥vQ?hçVKu?ïìN"Ñ w?wfÉà7Qè?c±{.ߋ>?wfÉà7Qè?ï6;!@ñ?ç«¨û??™=؛×áþ?ç«¨û??ïjv§±?}(7A^Ç?'±?Þ+
?}(7A^Æ4FGL J0558.8-7459¿ï\nWU3À=†r!…‹ÆÀ9҈u"ç[À<U¼ö•óó@ÚJŒÁo?ÿ¦>{f?µì>A¯!ì?±›!ô›?ûHÆÆ#@ê¬0Êù?‡'ÑTW+¿ãf$!Gx¿áÓ/M= ¿Ü+%Â1h¿âG¦Ý¤áK¿åW¥£"ŸAGNbll3FGL J0558.6-7459PKS 0600-749?ïýªyðti?,«Ý?2¬0|\¼g?,«Ý&?ïýFø!_²?P"í"÷?5È>õb«?P"í"ó?ïõõ¿x0?^í¶}¶¸?TŸÊm?^í¶}¶¸?ïâ¢ieZ?WçWó§Ö?mê]–š¦­?WçWó§Þ4FGL J0559.6+3044¿ã™3éd@EF%~>ÊÀ:Òn`/ë€À<Gfȋõl@"iôÄb›?ö¯•Ôèû?ÐWN»¤ÜC?Ú¾•Û}À@
¯H<¯³·@0&Ø1¿ïÿ£ž\w¿ïºÔaì""?ïþØ
b?åƒ)ë‹Ôµ¿Ü=½zÊ¿Ûö]"ÛšAGNbcu3FGL J0559.8+304287GB 055627.1+304251?ïªKb0<T?'ƈð@/ª?…m'sðë2?'ƈð@/ª?ï@˜ŠÞ:{?·ã87¹W>?—ìî¤8°†?·ã87¹W>?íħxûÓ?¢{8ÒNš?±ßÒÄ8!l?¢{8ÒN™?ïPâÁž(?‹ŒFÿIô?•ã§Ì=»?‹ŒFÿIô4FGL J0559.9+6409?ØìøÂ8¼@2èß?–À:þ¿yýòàÀ<´ZÐ0.œ@f™<ÒnL@¸<½°Ÿ?Ä8âʐž?¢Û=º?á°ê7.j@ž ÀêÁT?ïlËÀ]RÁ?£î˜àJd¿éól|*¿Î7UAPu¿ÝA¡
&¿ç¬?8¥
AGNbcuGB6 J0559+6409?ïéÒb?7k?d^U«|*"?f-Àȓþ?d^U«|*'?ïûŸšÏ?^Eù÷.?C¥–¾Ø?^Eù÷?ïå#_­?o?Å,Ð$?jÜ æRú?o?Å,Ð0?ï¾7tiÊp?g!Ê*nJV?€r"åcþ?g!Ê*nJQ4FGL J0600.3+1244?âã½5ˆsÀú¼þ"°À:$™Õ(»áÀ<` SÇþ@#^ÎÚîùr?ø4þ"ÅõB?Á*h‰VUw?ń8Hñ¶f@vQElñ›@–A¬rº2¿ïÿ='—t{¿ï=ÙìD?ïÿtµÍ­?Í'"™2§¿Çh—Ð¹¿ÞqG ¨"AGNbcuNVSS J060015+124344?ïÍçe¸ƒd?uêY©r'?yM#¾Nv?uêY©r"?ïêi'Ó^?'TÊI'×w?eý–Ø, æ?'TÊI'×w?î1£ä–9? 9R²>òà?¬åÁ¶žT? 9R²>òß?ïjwždG?ˆ}Ô¹'?'±3w8?ˆ}Ô¹''4FGL J0600.6-3939?àe'û_gÀ:6¦ڜ™À9Çü6FãêÀ<"š3Œÿ@»3j:±W@nu5¬?»S9¸ÞXe?ÉJ®yûn¡@'ÌÛæED@w‰µËÔT¿±gû;õún¿æJ	¾Å£
¿ë«ð«Ï&¿ëژÒÊ<пí¤Qƒ€R¡¿ïû´áô|>AGNfsrq3FGL J0600.9-3943PKS 0558-396?ç²i—qñ«?Çk¼îž?Л,Ñ©?Çk¼îž?ë}Ù6¯ñ?É-"í'À`?›ó%@<?É-"í'À_?ånµ¡½m?µ•,p­Fb?Õ""½æ…$?µ•,p­Fb?é"|ˆØN_?²k~8hhu?É®
ܞƁ?²k~8hht4FGL J0601.0+3838¿í՘ÃC²@›%,à2ÛÀ9{ôörÀ;ýxM·‡@ 1ÊRt?ÿHécˆÖ?³«½ž¹þ?°ўî˜$?úkIÅEïÎ@¯–×óF‰?ïð'Þh¤¿ÖÊ'¿âµŸSí½Þ¿×l=Æþ¿æ·E¡ŸÍe¿ÉJ›Ú'†{AGNbll3FGL J0601.0+3837B2 0557+38?ïØÔ·¹"?sMÌS£Ô?s•¤8#=å?sMÌS£Ö?îùˆØÊp?²}š¢«³? grsXþm?²}š¢«³?ï•6ß«]?†F^œ<Q3?Š²H(¹‰?†F^œ<Q+?ì¼þ¹×Ʊ?Ÿßlfð0"?º
1AÊm?Ÿßlfð0"4FGL J0601.1-7035¿Ãhɺò¥À=¡g‡Î•ûÀ8¹£¥Œ#À;è×Òª\@ñe¸°–@ƒ‡Ä"ÿ¯?£·¦J*ø?½Ò/ãšj@Fº z^k@pM6>«a¿ºŸ»Ç–×ó¿à*Iëœø¿æÖ`)5ƒp¿åЬÀ½ÊÑ¿è·âŸÇÛ÷¿ìT*Ÿ:î>AGNfsrq3FGL J0601.2-7036PKS 0601-70?ï÷Âë{Üâ?PátŸT¨»?Pz)F<›?PátŸT¨°?ïú/@{Ÿ…?]Ÿ–ù#šl?GBþê€?]Ÿ–ù#šo?ïʋÀà?~4µÀZú?zºÿòv?~4µÀZü?ïþQWé;?ë˜AH?*êlO-ø?ë˜Aµ4FGL J0601.3-7238?éázÎ5ˆÀ=‡·Ïå†À:øz§fÀ<£ñà'Œ7@\\sôC‰@âÃäƾ–?Ä wÚ,0à?§—j•J?åü~ìC@~q'´¿ë[þ*?ïô¤'*è¿ä?ʅʯ¼¿æ«QAç*¿Üá-â'Z0¿Î±k

pAGNbllPMN J0601-7238?ïü€ÉNj?:1;ûP®ä?;ÿQµŒ¬?:1;ûP®Ô?ïý+M…ª?XZµà¬º?6§"Ò¬«?XZµà¬Â?ïÏ·Tù¿Ë?z»×Zæ~?x$Uƒ k?z»×Zæx?ïî¶hMgÕ?RÂ%g±œ?aI—²˜*Ï?RÂ%g±—4FGL J0601.3+5444¿[`§BÓ¡@.=Ö[æÀ;7z)'ÉÁÀ<°œÉÏÂK@ Ñ6Œ.!&?ÿ€ì#ª)?ÉÝÂéI/?£Š¾ú?Ùb2z&@gï›û2?Ϲq%\0¿ìÕSïk]F¿¿c"OðÆ¿Û^'¢O¥¿ÛÞ9¿ëížÔkýAGNbcuGB6 J0601+5443?ïýW4—ìž?.2aÍ9Aÿ?5F[@›°?.2aÍ9B
?ïüÇÿ½a
?YI("Œæ?9À÷™'?YI("Œî?ïðx0e
õ?j÷䑜ì)?_Ÿ5äå?j÷䑜ì5?ïò¹De¶?DGØÏ¥?ZwÃ4"?DGØÏ¥Ž4FGL J0601.4+2320¿Ó-C -²?Íb±%&€À9Q¡/À;?‹!0Ò0@Ò.ϏÐ@#ë¤ÿ(j?Ãðç^HŠ³?ÊÛ9·†¿w?ÿãÿ¹‰#*@©5§¬¬Ç¿é¬¤G¿Òvǝ
"¿êçÓh'1¿èá?(‰â¿ç)\OŒ/N¿ïã²…AGNfsrq3FGL J0601.5+2309MG2 J060149+2324?â†Å¤…Ç…?Ðßpl¹?Úòt¶ôpö?Ðßpl¹?åÿœâ?Ô#j²`"?ÕðåÊÆ;?Ô#j²`"?ã»3~€ž?»Ã®œXî?Ùö‰™þÄ?»Ã®œXî?é4$‰?°"X£î?Ë/§ÇmÛê?°"X£î4FGL J0601.8-2003?z+ã±À3Ùä"sÀ::Ó8÷˜RÀ<L•òE,Z@±y]äâ˜@ir)Zl?ÀÏÔ©É?Áª~™8 ?ùA".öŽ@ÞR}T•¿Ï®2M"¿â°FŸ ¿é›H€w^±¿ì|¿8"†?§"Uür'¿ïýïŸ_¬8AGNfsrqPMN J0601-2004?ïþkÉ\ÅU?+ÜcêöG]?)Cj3ªµh?+ÜcêöG´?ïýÓaëX?OI&Èâgâ?1dð§Fk?OI&Èâgõ?ïÄÇ41™?}÷xÃú‰?}œeúg3Í?}÷xÃúš?ïùŸËþÃ?@så{qI?I€ÓŒò°?@så{qB4FGL J0602.0+5315¿ïŸ;˜>…@-%åр´À9{ÌÀ7"À<+6
Ä@ÈÏ»i£?þùLVè?®°ÀÁj‡Í?œt2¬Ðƒ?ð'޻♾@'Áƒ¢?æZºÌH¦¿Ô€'ཚ€¿á~•Üär¿Ù5_Þ7v¿ážXæK#¿ÓÂùå3ËßAGNbll3FGL J0602.2+5314GB6 J0601+5315?ïþ'½0^?  $V?'Ô,ú¹¶?  $V
–?ïü+$Ä@?^u\WœÊ½?>¦ßÝý?^u\WœÊ³?ïõ…˜ÙàÆ?_üŽzMÏZ?TôÎL>q¨?_üŽzMÏ>?ïû™ëjf?0%æ½?A›RVl2?0%æð4FGL J0602.7-0007?ïáÓ¡éï)À%»Åޜ*À:@x
Ә™À;Ê%o%QÉ@i€0¼áG@S7ë(Ø?Ê$ Eűû?ÃU6hFæC?ô²—,Ê@ÏÁZRÜÇ?æäíU'¿ÒãIüMmò¿éSe¢òð¿àÜ®ÙÄ­¿çãœA¿'ý¿ïÿð`OËðAGNbllPMN J0602-0004?ï¡Ž‹ëX?£j¾G?ËÎ.'"ó?£j¾G?îâL2LŠ?±åÈM?¡Û<Û?ç]?±åÈM?ì"lÚKH­?®W¹Ùì?»\™-¥º"?®W¹Ùì?ìB)n¼?¢#úå{?½î·¤Z?¢#úå{4FGL J0602.8-4019¿Ôw"¨UÞ¦À9÷±ÿÀ9HÙè>B[À;֞-}Í@MË°4z?ü¨zd×ñ?°ûe€Q7ð?º‰Û
¨$¢@
MÆýòÿ@çÖøj¿ïá÷ ³SÕ?ﻹ.׿àƒËÑû	÷¿Õ(šž&q.¿â«¤(hÔÖ¿æ &5AGNbll3FGL J0602.8-4016SUMSS J060251-401845?ïïl=…='?b²ÍáV?`"ÂzÂl¨?b²Íá^?ï…|"?¸CÛ0ö'ª?P|}›¬?¸CÛ0ö'«?ïmÔFRµ?&[ '?'Ew5¿	@?&[ '?îDÏh7äu?–íLÁvI?«³	|¸Ã?–íLÁvI4FGL J0602.8+6041¿å†¹'¯@1ÒZh+b"À;LN¢ûB+À<›—¸
@çט'Ã>@k¦ý/k(?ÌȆŽàÙ?·sÞt?î'ÿú Ã@p ó•Žr?ïØ+oðRä¿ãDD¾ÂH¿çÂ>hñ["¿ÝÛ«aïÿÿÊPË?ïÿý¡UûŠAGNbcuNVSS J060324+604009?ïû?…§ƒê?CƒÃuQŒ?CéaðV?CƒÃuQŒ?ï‰p9"?§ÿ2• è'?£ú=1·S?§ÿ2• è'?ïnõ ~™?…¢Ü) ?ˆ¤B—àY–?…¢Ü)?ïœ~vßw?yk6þ]x?ˆàâH"b?yk6þ]w4FGL J0603.9+2159?íU`Ml?¨˜,C;À9g l‡ØÀ;IéÁЈ@‡T>7É@·a*½C?·œ8°J¶¿š€)†G\?ãA® 9[k@	 ˒:*?âÁ?/À¸¿âÀ+i:V=¿ë¦¬ÂkIû¿Ñö0‡ÿ¿ëÄ®…¹èÄ¿˜èíû׸tAGNbcu3FGL J0603.8+21554C +22.12?ïÅé{KN?{&âê¬û(?}BpÚYd?{&âê¬û+?ïûGבÔ?sJ€Ùœ?Bà¡»ˆ²×?sJ€Ùš?îlˆnBÖ?›L×~Ç)?©7yßâž?›L×~Ç(?ïÞ$=º–Ò?bæ®]îé…?píá"´—¬?bæ®]îéˆ4FGL J0604.1-4816¿Ö[YÆKàÀ;}Oß;dZÀ:‰øg…JWÀ<|õÎMÖM@!SCÉÙR?ûêï,s%'?¿÷>….?³Íï6¯©?öêºÅ­@ú9lˆ>¿ï°OžMÞZ?ïüÅþ§e_¿ÜÀæå|ǿ܍üb;´a¿ÜÕ9BkàN¿Â¨Xú2ÍAGNbll3FGL J0604.1-48171ES 0602-482?ïÿEÖtÂ?!²qjg¸?E1g½qg?!²qjgÈ?ïýRmCA¢?Q»3Dâçó?5l•åòé?Q»3Dâçç?ïôϬG§>?\ñÈÆ»Ò?V`§p±† ?\ñÈÆ»Ñ?ï띲°.9?V"ÏW¶'?dbMOÑÇô?V"ÏW¶"4FGL J0604.5-4851?Ò­Td¾ñÀ;‰¹"¬TÀ;5£ÇeÀ<šó5í"@:^}¹¿)@{\ÚÌiÐ?Åícۜž\?‡5ÖP¯	?ÁÊ'˜˜"@ftá~_¬?ïõœdO4ñ¿å›	Ü!Ôf¿éë‡ç`Í¿ÝÖÚhµÌ¿ês€€C¿»4.A2³AGNbcu3FGL J0604.7-4849SUMSS J060433-484947?ïó	̎³õ?\™
Ftæ?Yìf☾?\™
Ftæ#?ïþ4[è?'?DV—Rçöè?,ºA|
'õ?DV—Rçöä?ïÇé)[vN?}L0´üu?|kRDÙO?}L0´üq?ï÷SÃ(EÇ??Iò=4€?QXy¯tt??Iò=4˜4FGL J0604.8+4411?ß/ì0@%Èù±1eÔÀ:ecãÔPÀ<Ȓ«hÏ@:"çÛÇ@oê#èù?Ã×ã–½Ç ?«M-5?åŠgAؒ~@˜Õl²?Ûú"•üV'¿æ»`(^ÃÛ¿âèìô,¿ê§Š$Ô¿æ²^âc¿ðAGNbcuS4 0600+44?ïû{æs?AqX|¨R:?CÎf3äÜ?AqX|¨RC?ïøÚ²5®?n³ïì;ü?L—¥7)G?n³ïì;û?ïÉf\,gÚ?zq°@.Ë?{LÑéÌB?zq°@.Ë?ïÚx&S&?\´-!Ï?rÃìÖlùy?\´-!Ð4FGL J0604.9-0000?ï U'¿±À$§ñQçSÀ9Ö¡Š(ãNÀ;ëŸ+©Ñö@ `|°Ä®?þŤðñ5?ÁÇÓ(["Ð?Àöh½ÕG@Õ%`â™?úé!>"l?ȏËåq3t¿ãP´î‰µ÷¿ÛžgŸ —$¿àÕß?Á#¿ÍÎùÁ¢w¿ïÿú Âî'AGNbcu3FGL J0605.0-0000GB6 J0604+0000?ïÚA%p[?v#Y¡·[?rßmGÒŽ?v#Y¡·[?îdåeK?»]íZÎ-?©¿q©«Ou?»]íZÎ-?puc?šI§í–#š?¦öøø©Ö?šI§í–#—?ëWå"Ðϵ?ªs‹QU$Ø? i°¼Á0?ªs‹QU$Ù4FGL J0606.5-4730¿ìßà»qÀ:ò|ᛑÀ:iƒ¾f½À<~)gØVn@¹_÷·\"?þSó?ÀgX>Zƒ¯?Ä5â:[€@Jb#ᆘ@ÿ8¯ÉÝ¿Ê~ÆÀï?ï†va[9¸¿ØBµ<u¯¿ÛlÛ z3x¿ã'ÿýPοç¸u'8)AGNbcu3FGL J0606.4-4729RX J060635.9-473001?ïïðàEõJ?`«ä
**d?`º
·6?`«ä
**j?ïõèútC?wV*':»?T.ùw÷?wV*':¾?ïÐ×í(s?uúÄeéŽÔ?w"	|kÆ;?uúÄeéŽ×?G½Ý?zžʦÃ	?ùÐ.ˆê?zžʦÃ4FGL J0606.9+4402?瘝w'¹@&SZBkµ[À;ˆ²køvŸÀ<¯
¾Ÿã`@"vJâ§T˜?àÖ`ÿõE?âÌ|ý?ïÿÿ&¦³@™xâií@žÔ2FÏ¿ì?2_Μ±?Ûìû@}ž'¿æïa¢1n¿Æ`¯Z9²?¿ÒČ¿ïÿ̞©£ÓAGNbcuCRATES J060650+440144?ïß%×r?xxÊã"e?pvmF¸Ç?xxÊã"e?ïæfóûõ?…&sêá?ip™x?…&sêà?ï.مgo?'€Žœï'?š$ÏS²R?'€Žœï"?ïâM[4þ?pcÊ3'¼?m²ú¤Ëà?pcÊ3'½4FGL J0607.2-2518?æêÐY²\À4mÙ ð¥ðÀ:ñe9?¼®À<­¢pØ°0@ Iý?üÿ¥·µ
"?ÌNÖý¨7?ÒûG¿1X¾@*3<m@î" ÞÇÌ¿ïÿÝÑô?ïòÑ®³Ý¿Ì°B'—É‹¿Ô§â݅W¿è…ÀsοÆx øóò+AGNbll1RXS J060714.2-251855?ïîMât+?]
[Ò¤zr?aﲋÒÎ?]
[Ò¤zq?ïÚSD3µf?Œ$šê7â?rÖ]æ%M??Œ$šê7á?ï	K¿g5?•Vo,Õê?žÖˆ
ó ?•Vo,Õë?îüU*"£I?Œs¾"åâ? :­VÅËd?Œs¾"åâ4FGL J0607.4+4739¿ä"oCú˜@)»ZBkµ[À8KÅPÉÀ;‰†¶hz@hÛ!yL?ÿ묋å?Ÿžöaù?²î˜àJd@Éé^ÓÊî@€9Küï?ä·¬ÿýѧ¿Þ­€×*ô ¿ß–7D9ë´¿Þ9p¤'Öµ¿ä,™¦5¿æ%¢HZãAGNbll3FGL J0607.4+4739TXS 0603+476?ïý|¶hì?*¶={9Ë?4O<¸¤Û?*¶={9í?ï×Ù"oq?'#mÔãÉV?tnÈGrÙ?'#mÔãÉU?ï¿çò–s?…:> "ß?€9†Zcˆ?…:> "ß?ïµÄòA?r?hSNU¾~?'ŽÃo°#d?hSNU¾}4FGL J0608.0+6721¿å/"ƒ}hd@4ßH!ÄvÀ:É¥Ð߁À<rÁÄN¯@Ô®rC¿G@e²€fÃ?·_ïÕ?¶O•¿ol?ýŒð=ë@‹ëëv@?ïþ¸*¥¿åڀ¶–*¿æšmÔﱿç
ýQúÊ¿éOt¢>XÖ¿ïüßÿÚkFAGNfsrqS4 0602+67?ïýàù~ß?0ä¾ð²"m?0ø4	ú?0ä¾ð²"m?ïúXéàô?\õír?FœXø+k?\õít?ïȚëø
?y%B¦ÞÁ?{²þŠú"?y%B¦ÞÁ	?ïùK:<B?8ÌL]Šß?JÓÞöÙ?8ÌL]ŠÞ4FGL J0608.0-0835¿áXÕõÓÀ+-{cM­À8z!ÛòÚÀ;gUá³äž@Vä£-@ÝÛ?VW?§ åþ¢û?²#ì€ÏÚ@M­àx{<@­þ/Eh¿É]úºpª¿áé1â¦'ò¿å¬¬›ÔÝ=¿år|õ$®¿ëÏY¿Žö¨¿ã‡%Ž/AGNfsrq3FGL J0608.0-0835PKS 0605-08?ïú&òÅÿ]?D¨Q}V$?Gd4è‹$?D¨Q}V?ïúunIÀ?h@v|3!?F*G¢Øýö?h@v|3!˜?ïYþC.X?Ž|8£Jk?"À7š-õ?Ž|8£Jk#?ïþÈøìD?5°p>­Ð?#psÅ;³G?5°p>­š4FGL J0608.1-6028?è:ñªežÀ<¡ð†nDÀ:+>WS£ìÀ<
¢"ú¦$@Þ)=Ðñ@T™Â´E?ÅÆæXäóŠ?ÇU¸a°Ê@¥á¦x¥@Ô&Z²©
?àî姏&¿æf¬![š[¿éq+¼FlÌ¿éê šª;¿ïÿøþÙå9?äãÀEçAGNfsrqPKS 0607-605?ïõ¢-§Ä?VDÐ[Ö?T»¥Ò°x"?VDÐ[Ô?ïú±ùÉ?f*k¹]Î?G8 Ûè?f*k¹]Ð?îúÕx<ç?""FÞ-ǃ? R¨x1€?""FÞ-ǂ?ïåý+¨j¨?\'Ž;–Y?jÔW•X?\'Ž;–U4FGL J0608.1-1521¿ã~Gƛ7À0aóFí$À9²L‡À;ãIâ¢!@ª<ANÔÏ@aÏBÈÒl?­Q4¿¿	?µåê**ËÜ?ÿG±õ°ñ¥@ô÷ή#i¿ÐFŸ ¿â-¸À%t"¿é£€}"Ô‰¿æ5v•ˆ"¿é"|žâê¿ïÇõAàõúAGNfsrq3FGL J0608.1-1522PMN J0608-1520?ïý¦{ÖH?0|sH7ƒ?3òÌ!M·£?0|sH7ƈ?ïý"o=£?S	'¼è‹H?6ì†çWv?S	'¼è‹:?ïžù`ƒg?ƒMýN{͗?ˆA¾§ß&"?ƒMýN{͒?ïÿ£Ë˜>þ¯«õn½?
<>Z†>þ¯«õn 4FGL J0608.9-5456?éo-t<À;Þâ¨dªÀ9·CsóãÀ<^ÄÞÁÁ×@Û]ˆœFG@""³º­?¶æPV"œ?Ø*ƒ·/,@ö"aKts@[ûÎíäJ¿â F\㕿ãíÝÞÂî}¿è\…qÄhz¿ëZ}ú×¢¿íÓø:8á¿ðAGNbcuPKS 0607-549?ïþ¿×a?,U´òû˜?."‰ï	ã?,U´òûÉ?ïüہîÓ[?NÓùÓä%¹?9#ð‰e*s?NÓùÓä%³?Óß¾â?;a1Ÿž?ˆ•ËGs?;a1Ÿž?ïó¡Ý'§?Jb¦êe_?X¼Dú±ô7?Jb¦êe|4FGL J0609.0-2219¿íTÊM‰OnÀ2ñåÀ¹™À:ãêÀӚFÀ<x
œ;4‰@õ¨ä_@'‹vÁ?Ò:og–è?Õ£(c¡e@°ÄXŠÑ@	ªçŸ¶ê?äEôî¿äb¼ÃjM|¿ßM<+¬¿á¡4x­'¿êƄ^I¿ß·$¥Ñ¶AGNfsrqPKS 0606-223?ïí¹}HÂó?b"¹æ8G?bF'·=»?b"¹æ8D?ïüiœ4áÈ?^Íy¸C?<³XñÈ4?^Íy¸C?î—Už\ª?šù±–p?¦Š¦5^±?šù±–n?ïÈî^q¸?eº1€Ð§w?{ˆñPÇ#"?eº1€Ð§s4FGL J0609.2-0247¿ïʋDÈΚÀ%Q|=h@[À9‰PÉSœÀ;Êrß­*@ 7QŒºŽ?úºܓn?¸õÜ»'M?LJeºnü7@«3¥Cò@˜¡˜–N¿ïÿC*!<?ïýûþé‹¿¦`ʛK¿ÔŽUëæοÚbX"üS£¿è'kr>á½AGNbll3FGL J0609.4-0248NVSS J060915-024754?íÞáž?²¾?/"K½?·ùÀ÷3?²¾?/"K½?íÊÙ^Œ	?Ä%_Ö³ú®?±©5Ÿ·þ?Ä%_Ö³ú®?鮸g—"?°e€yÙÿ‡?ÉEÞa£{?°e€yÙÿ‡?é1U"ÞZœ?±(cº²?Ë:«t†•'?±(cº²4FGL J0609.5+1402?ãÊ­ò¨À&ü›ÇqCÀ9¼ˆ\ZsêÀ;P°Å/Iš@×r'¦
@.—ÂÿÄq?Ëaë¼?ÍÍړßÆ@yŠ˜?ûptgÊ?ïkcÉ€?Ñ´GDãù¿çt÷Ãñ[ø¿éxv¾ù$š¿ãºàŽµ:¿ï÷šÁ6ì{AGNbcuNVSS J060922+140744?æmeÀÞ?ÌHÙJˎÞ?Ó%4~Cù?ÌHÙJˎÞ?ç62×û˜œ?Ñ>m—z˘?ѓšPÎÇ?Ñ>m—z˘?âéӍég?¼Â"í$	Ì?Ú,Xä-Ã1?¼Â"í$	Ì?Ú9AýJ7Œ?·ÎßÜàÙ?âã_Zä9?·ÎßÜàÙ4FGL J0610.1-1848?êÓz{
À1Sü¹#¢œÀ9Ü36ÌEÀ<(!à$˜f@Ž±¥ÿÙj@SI€C‡?ºbe¥Ì,ê?¸NPº*?ýãGG½-ó@
âmúy-¿ïΣ Öå*?ìû‡_Û1ê¿äßzïŠf÷¿åu{aöD¿å©ø¡çÆοïÿ"ÞïAGNbll2FGL J0609.6-1847PMN J0610-1847?ïøNU¾ž?R;Q4š¾?MúÆ©…ž?R;Q4šÇ?ïù%9Íä??qW7³%±Û?KkÈo'?qW7³%±Û?ïD:K‰°ò?"_µyNý?—x¶ŽÉáå?"_µyNý?ïËcê¨b?kK¶¦¸D?zN
«ýN™?kK¶¦¸D{4FGL J0610.7+1656?¬{ïñâh¡¿ð%Q(ÀBÀ9&ÞßôǾÀ:ù^³ê}¸@ÀØNá£@6þ.n¨T?ÏiE~d^ú?àó°0´Ó²@ê¦ÒgA?ôWTБӿ̼°à]"p¿áO^AÔ¶¦¿ê¨ªxäî,¿ë6Èéé¿ð?èÞ¸AÐYõAGNbcuMG2 J061020+1701?۠Ԃ'\A?ÕµZÆeq?â/•¾¶Ñà?ÕµZÆeq?ÆSf'ÕL†?Ð<6X¼,W?êk&v
¬Þ?Ð<6X¼,W?ÛgÄ³ú?¸§–+?âLù¦v?¸§–+?c(pS&Ç?UxžÂí?ïì׏¬Ù:?UxžÂí4FGL J0610.9-6054?q.‡À<TÔÜeÇÀ:Vªñ°±äÀ<%ÚV"K"@Ës0yE@|#ßÙ?ÂMò?¿1ãÁŸ¶Ù?ø¿}Xñ3@
5¨µv	¿æ5(¡ù¤¿à	+ÝÔ\
¿è'Bbûù¿èG"žy_¿å#—´½¿ïÿ¼C͈AGNfsrq3FGL J0611.1-6100PKS 0609-609?ïþ¬Šê?'Ù-W'‹?%7V/1Q|?'Ù-W'Ž?ïýZÅj?PB"2Î5?5/Ñ×\­¦?PB"2Î)?ïÉs«Jé^?x
¨/?{F*Z‹PÇ?x
¨4?ïçU"9?YÇÇìv²?hªêlÆùh?YÇÇìv±4FGL J0611.1+4325?ïëÛ×l¦@'"ãq*À:ù»9À<Bˆ4ˆ@ «*èáÖI?û¬½³TUÃ?ÀA+‡‹O?À`Ò}»ÂŽ@*§Xžý‡@÷˜OŽ?ï9Õÿ{u¿㒰qLsv¿â}§Ë‹"-¿ÍzwëI¿ßõu|Y¿Û­A—$AGNbcu3FGL J0611.2+43237C 0607+4324?ïîŒ1H1?`Ÿe
–v?asηäÎÒ?`Ÿe
–q?ï'uó^p?°"Š\ìY?œM±A"2?°"Š\ìZ?ï"9ƒŒ?Š6ïþó"?‹9ñŸ:Ý?Š6ïþó"?î>2óÊ´î?'v…F}ÀR?¬ÐÃT±?'v…F}ÀS4FGL J0611.6-2712?³*Ù‰q2À42®žä\6À:TWLíï\À<~vQ•ôÉ@®Š5x‡Ñ@HÜè£Ã?ÂE³ÆkŠ?½DÙMäa?÷Và·e\@¨AƒMÓ?ïÿÂÝ_¿åeƒGG½.¿å»;ÀJˆd¿äꨠÀ€¿ð?ï©·¸iAGNbcuPMN J0611-2709?ïÿºbÊ÷Ã?æc?gMBPó?æa?ïþ_#Ã:?Dlù×ØH£?*
ÃÎ\T²?Dlù×ØH›?ïÑín•?|ü[?w~‰Hµ}I?|ü[ý?ïÿLd9û?¶ÈÏ,p?ösxÀY?¶ÈÏ-}4FGL J0611.6+2803?Ä´o
´@Ð]{ZÀ9ïËñqÈÀ;Öè`·Ñ@õÒö\")@æuš¶Ð?čaûÁ?ƨºžÌßA@ÓrSÍÝ@ʺˆýj$¿à4³eó?Ö÷PÄh¥0¿ÚÞŝ®|*¿ä2>@­o¿è¬QéØ¿åd¹½üOqAGNbll3FGL J0611.7+2759GB6 J0611+2803?íã
¢Å»?°¤Î)™®?°ç'ïYÒ?°¤Î)™®?ïݹ…¥Ã?‰!¦¢Qi?q#7½-¶?‰!¦¢Qi?í¼«áÁÁ?¨Ïݑ«µé?·
 ññö?¨Ïݑ«µê?ï²@¢?… š¤B…?ŸI¼_—ë¤?… š¤B‡4FGL J0612.5-3138?îÍ4¸ÖîÀ5Œ
9>åïÀ9覨uÕoÀ<5Ûèɂ•@¸ïË)Š@îòžîm1?¶1Õ i"(?­õ}FLÒ?ñÒ±HL@³×1)Þ?Ӭȵæ×:¿äayÝf¢÷¿çéµ²¿èfu 3Ä¿æTg–NÝ¿Ø­>2­AGNfsrqPKS 0610-316?ïýkú±!?.'8•&"?4 *v÷?¡?.'8•&"?ïþ-?Îd?IØÓ»
ˆ?.Ý,¶U?IØÓ»
|?ïê5ãÀ×?c¶rÔáÆ?eÊô?(Ú?c¶rÔá¿?ï÷ù³‰äþ?>sªx™ù?P˜ì6?>sªx™øÈ4FGL J0612.5-3934¿³˜äÞâޑÀ7ùrÿÑÜ×À:ÒȏPj|À<a3œå~t@蜞¶@M¹â}q?Ô%j­¥j?Ã÷‹<^«?ìJtÎ6/@ØCÊZ+Æ¿ã<~֟´f¿èâzžµÍ¿æ+@àðÆ&¿àó"aÌMÌ¿ïÿÃF1=¿åœúÂSw AGNbcuPMN J0612-3939?ïþû£µG?"lE;H? EÄ«?"lE;!?ïþJS:B?J}[aþb?+ZÌ^ÝÓ?J}[aþr?ᅮ.îþ?ò".3Ú?€>4D@¼?ò".3Ù?ïöêÃÙó?D|÷i •F?SÒ*xL?D|÷i •A4FGL J0612.8+4122¿âWÉ] S@%ÚËB‰ŒÀ7ïßlÁÕÀ;YKHÓ®h@wáú†n?ýQýýûC?" ç^Ñû?»Ù¥ß^[@ ¶ñýÞ½@¤e¹˜<¢¿¾+"˜†I0¿Ó™ä'¡¿Üýüdêæ=¿Þä[^Ëg¿ä	ó‡K¹¿æ°T%òAGNbll3FGL J0612.8+4122B3 0609+413?ïÈ5Ù£+?~VÂm
bS?{å~®jU?~VÂm
bS?êÛÍ·l™†?Ðõ[9Œ›õ?ĐÉ"M™ä?Ðõ[9Œ›õ?ï&‰;:è?˜p3Ýph?›.؝8¢Ï?˜p3ÝphŽ?æwþcÓ¸
?¶ Á0–Ä?Ó8Xí?¶ Á0–Ä4FGL J0614.8+6136¿Û
(l–Ó@3Ùb¶®À: èj¸¿À<l³â;ë@35í!Öê@ž7€ŸÍ?Ë<b[ê·n?ÎWÜö:¯S?ûUÕ¤â¢ø@
8Xöh?ïˆ;¾/á¿Úf2CÊF¿éƒ<€8õj¿ç)L?Í¿ä됧'i¿å"ߨò}AGNbcuGB6 J0614+6139?ïÐCY¥¸ø?|"I«§z?wÞS-#"3?|"I«§|?ïùEà@t?h($("‡?Jèªþ2˜?h($(""?íÑÊrŒžQ?£ÎÌÚÞ®?±q¬k›
z?£ÎÌÚÞ®?ïã6 ón?WÌ—·"Î?låÉß'ÿ?WÌ—·"Ø4FGL J0614.9+2426?Ìԗ²,x—@§TßÔÀ:‡²Â_‹À;ó
8h&Z@´•‰¿‡?û´Õ)' ?Ø쒅(Ht?怸!D@X`~Åؽ?þ®ÓdìhÉ¿ïü0g¦ØF?ïüÕÞÄF?™óMa[¿Ö'×ÞxÆ»¿ìÛU%ÌB¿ïýCŠUAGNbcuGB6 J0614+2426?æec_w®?ÊځÂú?Ó59Aâ¥?ÊځÂú?ØI7~"3^?։‡¶p`?ãÛd@µæQ?։‡¶p`?âê5c^÷,?¸ÃÞH^£?Ú+•9B¨?¸ÃÞH^¢?ݳ	E)Ü?¹¿Þ%¢—M?á&{]k{'?¹¿Þ%¢—L4FGL J0615.3-3117?íQ®žÛ}À4ÛaE•5‡À:Uôÿý²À<hÏ(ǟf@ú¹žßZ@Ò[YÂéõ?½r¬Dìï?¦¦˜ZªEŽ?ç/œÛmy€@Á–vú]T?ïþ?üšE¿æ¡³^f½¤¿ã&Àþb¿áSÅDBO0¿ãÖàµwF¿Ýš_ý–™4AGNbll3FGL J0615.4-3116PKS 0613-312?ïÿSm¤æž?ç‰zmK?'Kc,-_?ç‰zm=?ïýþœé°›?T§Ó÷':?0²{&Ñ?T§Ó÷'B?ïù'"^¡%?X2{ðÚçx?Iõî…{p?X2{ðÚçƒ?ïôD|œWÏ?Bÿ›¹»/?WwÇPc}?Bÿ›¹»/ 4FGL J0616.1-1732?Ø0eÄ6À/j;Ýü À;~ì\µ½À< Òc傦@!÷ŽsuÃ|?öښéœ?åö\å®›?Ù¨Ã"ð?÷†D·%?þўEzÞn¿ïþ'!€-b?ïôJõǗÚ?Ñú±AV¥¿Ø2ÒûÄ¿ÛÓmE'ÒW¿Ü  0÷ïAGNbll1RXS J061609.5-173313?ïù*\ý•?G¿míÇ2?KVÐ	¬V?G¿míÇ1?ï÷c>:nË?pÿ˜ê-Å?Q9ƒ‹"h'?pÿ˜ê-Ã?ï²àú?'Ì¿Vø?ƒ}øÿÁŒ?'Ì¿Vû?ïŒ^°b?{Á]·'-?Œè}Óà'v?{Á]·'*4FGL J0616.7-1049?Ûeу€;À)"Í[h£À:N.a<[À;¢ûú·Á£@G˯ÁN>@ãÖáù"¼?ÐÄR1ž‰?Ù¦žD¤Ù@ñ©áyñ@—rÄÔ?ïÿéà
v¿è@‡å</[¿ìcMâáâ¿èá}ÿ	_û¿ïÿÿ" 5•?ïù*ù¨ÍêAGNbcuPMN J0616-1040?ï¸+Y´9 ?'ä«i0y/?õ)'ñ—Ò?'ä«i0y0?ê
•w0ì÷?Ë®†­Î?Çɪ#<L"?Ë®†­Î?æ9{a1-¹?³ÒÕ2:Ü?Ӎ	=¤Ž?³ÒÕ2:Û?è.G1ûy?¸õ¡*"8?ÏFã9ø?¸õ¡*"84FGL J0616.9+4340?íuôÙè'@)<ù;À oÀ;ÚÂXՄÀ<À­°i@"—¤}£Cç?ù¼'«A?Ø	zg¥*Ç?¼O ÒÀ?éÙ? ý&?÷Š¿Ì‰0¿ä¿@OÁß?ï«ù4㍿ٸ)|¦Ù¿Ý&c–þ4?"™húÈç¿ÜºÉ?$AGNbcuGB6 J0617+4340?ïý®åf?1"IÈ ?2ˆ×?$Î]?1"IÈ ?ïÚD•@?"òš"ÅM?rôݵ_ô>?"òš"ÅL?ïÞ/LÛ¨?r­âK»L¿?pèY'+à?r­âK»Lµ?>ÇûŠ?}²áWÿ±?Š™pNm?}²áWÿ®4FGL J0617.2+5701?î*
Î
@2ëáe
FÀ9I"žˆÀ<(ØåßÃJ@‹AÑ܁ @a´5&Rz?¦DpÈ??§_™m¤É#@"'Æ@
Ð-µý­¿Ñ£ˆ{>1¿áZºÌH¦¿âA¬=
LŠ¿Ü"ëø>ø¿åø| µ¿ã^'/éAGNbll3FGL J0617.2+570187GB 061258.1+570222?ïüá/pDY?3	ê,¡AV?8ö"}ÝA€?3	ê,¡A?ï÷í7¯vá?b¬è?P%¡=$?b¬é?ïðxëìÕ$?e
w€ã¨Á?_(&U¸,?e
w€ã¨Æ?ïå	ȍQ~?X— Êp?jö7r®'ž?X— Êp
4FGL J0617.7-1715?ÐíÊµRiÀ.!6ŎêêÀ9"#rËÏwÀ;Û¢4rÎT@‹-á
¡?üœ¡ž¥r?¶¢?/•ÄÎ?¼ÜÎ!¶‰@¹ÍÄC'O@v]ÃՂS?ïã3@Ÿ-¿àÅã~ê읿ÝÈ輗u}¿ÖÞ$Þ[À¿ÜàA>
ׯ¿ç=ý¼ƒÔAGNbll3FGL J0617.6-1717IVS B0615-172?ïñ¸Ïf·3?[Iœ´?\Ža2'œÍ?[Iœ³ý?ïÜËD‹Äb?"dªÉ‡e?qš]ºϲ?"dªÉ‡e?ï³·Õ*+~?"¥‹"q½?ƒ
µu Œ?"¥‹"q½?îò`žöOY?ÃMg\°? Ùö›
]?ÃMg\°4FGL J0618.1-2428?ê""°¤À1՟+©ÑöÀ:Žîr9€À<Q·åž@ñü"up@ÅsS6?ÊvófêoË?Ê\o—'ƒP?ûëlË@5'éþâ¿çzŠªéM6¿Á™Ãàêç¿åÈÜä.¿ã"I,«¿íÁÍÊùö¿ï‹›ÿûMiAGNfsrq3FGL J0618.2-2429PMN J0618-2426?ëºAÏ^s!?¹†q">Ú?Áø†3~?¹†q">Ù?ï¨{|a7?ÕÛﹶ?…á ûg±á?ÕÛﹶ?ëæ£ÚÃr?¨PP'ÞÝg?Àep"óÂ9?¨PP'ÞÝg?îžrŒÀH?'ª¢²~û3?¦ß3û~?'ª¢²~û34FGL J0618.9-1138?ï»Ê0Oµ9À(Ӝ"öœªÀ:%'ºZ'À;±B¾ÁqO@¸w¿T>F@	1)Ì?Ïåwh—C(?ӊ©|:¹@W
"˜±<@
¯î~Î<¿ÞUµßJ}Ó¿Ù@½!Þø¿åÒ!ÀšŠ¿ëò9Wÿ›¿âÔrþ¥7¿ïÿ­AGNbcu3FGL J0618.9-1138TXS 0616-116?ïæ¶?Ùz?m×ó~š?iIëÀ&"R?m×ó~›?ïób²¦e˜?uSì˜×?Y:š³4Ò¾?uSì˜Ø?ëÀoš!´à?¦ÇG­9¦?ÀþA—y,{?¦ÇG­9¦?ï«rÀ|Ä?sL­³Öå?…<ãOàÎÂ?sL­³Öæ4FGL J0620.3+3804?ì¾Ïµª"~@%|L7æ÷À:5ÉæhÀ;™4A@3X¡¬¸…@#ŒÚnuÿ?ÎP¹ŠÖ³?'£7'3 –?Ñî¼t@`­Eîé?ì8npöã!?Û{ļ²ù<¿éÓ¯ºmO¿æ(ýð[GN¿äêîU³¼¿ïÿöZdÐdAGNbcuGB6 J0620+3806?ëøy"µMß?¾J—Ó¼1?Àí*ȉ?¾J—Ó¼1'?íÝ/â¶ì?Ɓ™×s¸ƒ?·™€êH¡?Ɓ™×s¸ƒ?ê)ۂ†!?±p€bË#ò?Ç[ 'õçx?±p€bË#ñ?ìÓÿ­å
?¤àoß²J?¹`×•?¤àoß²I4FGL J0620.5-2512?î}2•Ë9ŠÀ1™ºç£À9¬6KìgÀ;å &5@añµaÌ@]d_%)…?·ÈG¾àù?Ï°%1½½@WƒPù@KF?jú?·J@€x¶J¿ã*óÿ@½_¿èYö|É¿èæ	ITݨ¿ïÿé{2¦¿ÓÀâÞ±ü'AGNbcuPKS 0618-252?ïÍ5 '?{rÁCX|?yeoì{ð¹?{rÁCX}?ïï¾{ˆŸ?|Ùõé}¸?`A"pw^ö?|Ùõé}¶?젇ð³@°?¤‰Æû#¹?ºûÀzeú"?¤‰Æû#º?ï´	ò‰?qsiØس?'ü<}ƒ]Ó?qsiØØ·4FGL J0620.7+2643¿í¥ÄŠ+þ@¯^AÔ¶¦À:¡…}'ãÀ<E-5Ã0l@#XÅq8Ò?ø‰{>d¿?ÀÜ gS¡=?¯pÐDÅ?ñ&'+½óì@<HQRƒ¿ïø½Ÿ¤v¿î¿ >ybm?ïÿ!ž5_³?xõá)a^{¿à
Ç9G¿œô"'|êAGNbcu3FGL J0620.4+2644RX J0620.6+2644?ïÿsu†?
÷ möÛ´?œ±O.?
÷ möÜ ?ïñ"yâÜe?ŠöˆðUp˜?\÷:G6?ŠöˆðUp™?ïöt²mž?d‰	wܶ?S›%Âij?d‰	wܹ?ïòòÃý§?PŽD6YÂÝ?ZyÀ³Î?PŽD6YÂà4FGL J0621.2-4648¿îis¿FFÀ8]æ?À:×Fšï/À<{«?´Jö@€Ñ¯	ÃM@Ò>ƒÉM¼?Êõ°kϲ?ÀôºQ Ä?ïü"à՘M@Éf'0CÀ?ïԉ>؂ã¿å©é]|2¿ç)y
­Øì¿ë);b¬'¿ïÿ¾ú¿±€
A/šAGNbcuIVS B0619-468?ïýãÂ}¹$?2Öá«·mÚ?0áì6ã?2Öá«·m"?ï¼Ã°ªCÛ?•2±›³ ?€ÏÕoý?•2±›³"?üê¤?"ÆÔðÙÈg?R€Å–²?"ÆÔðÙÈe?ï^±q15?'PqÇÖÐñ?")ÑÝÙÙm?'PqÇÖÐñ4FGL J0621.2-2213¿éãÀÖõÀ0LY§;BÌÀ:¸
!Áñ§À<vžy_g@"SCôÌp@b5deÛ&?Í/ÉÜ­j‡?Ï'쮤@=–é»ðÜ@Æi'wâ?íÌÙ,V  ¿äˍ Îí¿ã§".οâ.0y²É¿í*áã¿ïº«ÍxÄ7AGNbcuPMN J0621-2213?ïá<¤9•_?n'qVóàØ?nÃ[Æj¡5?n'qVóàÚ?ïòY3e]?€¬øúî?[M™5Eј?€¬øúî?îH¸§9N‹?œ©]p7Ï»?«tuŒkK?œ©]p7Ϻ?ïŽe®{©b?sX|›v•Î?Œf"a§q?sX|›v•Ñ4FGL J0621.7-3411¿ï°,øùÏôÀ4"D€bïÀ;ö¤À<‹S+ ?;@ L'Þœ?þZ˜⚔?ЙÇ|Uæç?Äx†$?òbI$.?ÿ‰®ww/â¿àÈA§õÓ¿î1­ÂEŠN?¹ú[?/¯Š¿Ýkq}›·+¿ãQf™'
¿âõÚã1AGNbll1RXS J062150.0-341140?ïü!'ñ^?6»€ ß{?>ópu_?6»€ ßÈ?ïüNõÙ$ð?YA'lZ©?=ˆQ6؃?YA'lZ©?ïÚèÒªN?t˜ª¤ôÜì?r÷‹–ªÙ>?t˜ª¤ôÜë?ïÆâoÏn¢?e×Vö…Ò?|ŽÈH®Ý?e×Vö…Ó4FGL J0621.8+1746?á¢gÆíl?ûyŒ³Ø	AÀ:¬¬ÊÎÅËÀ<Û£)eT@!å°²9ùv?ýË?.9?Ìa2µ^ñþ?­Í bSºÆ?áxg_µ0@<¹y]å?¶ÁŒ@¯aq¿ïÿ…ãp?ïáeáhö¿áQÛm¿ÐÄށU*)¿Ù\+d‡¾üAGNbllRX J0621.7+1747?ïþ=WB{?+র¿"o?,.ú‹ØV±?+র¿"|?ïùöTó–C?rԖÁþïW?H&¬1¦ò5?rԖÁþïZ?ïå¥Ç±{Ý?xô§Ø¾?jZ8N"#C?xô§Ø¾?ïø…,
Ò?D€œÛ˜"g?MëOː²Ž?D€œÛ˜"4FGL J0622.3-2605?ÎÐ6À1ŽPÅë1<À8w¬-ðÔÀ;¢ªùš‹@ûNuÙËä?ý÷dñ`¯?¢¡È€üƒŽ?
YJI$a?úbxÐÌ5Î@8xé@¿á䥜[d¿ØqCå+B¿Þåe_€C1¿ÝÔY¨‡s¿ÚðÁ^.´s¿Þìþ¢˜œAGNbll3FGL J0622.4-2606PMN J0622-2605?ïþ³"ק8? ñw†ïŽ³?$Æ…Œ~Ï? ñw†ïŽT?ïüÒ
±ª®?Uë»L~e?9o'rª"'?Uë»L~W?ïÞö«y?yKï£ì?pð"±*C+?yKï£í?ïÿ?oZG?ï@ÄLÃ?½÷$Q?ï@ÄL4FGL J0622.4-6433¿ãp¼SUÀ;bÎ-±êÀ:»ƒÑÀ<W0º²îÕ@zô»Ô,@¢¶®}Vm?ŝßN"¿°ÊkÞöE?å"Èy€õ^@'~øƒ‰ã¿å@¯½ÈM¿æäÚ_²m%¿îA¨v¬.È¿ÒÊrŸ¯³6¿ÐgÕÒ/¿ïýßßy!ÕAGNfsrqRX J062308.0-643619?ïýIϪ??˜NþÝ?7o±'¶‰??˜NþÝ~ñ?ïìR€"t?…T÷Bûß?c­o{ŒÅ?…T÷Bûß?ï‰ÁÎÙÈ?†¸€Z´?¹ÏŒI­?†¸€Z¬?ïòò6j`Î?T±\\Ö?Z"+>cš?T±\\Ü4FGL J0622.7-4141¿Ð…3#"À6¸¼M"ÉÀ;Ć­-ËÀ<ØmSÀqu@œêxÚ1d?ÿ¤2‹m‡?ÈeŸA#`Ø?ÛKkä)µ±@g ã¥Vf@ãNòï¿ïÿûÎBÓ?ïÿÌÐJ†¿ÝÌË_ºOÈ¿âqß«Ì¢¿ëäò}¶d+¿ïÿå]½JyAGNbcu3FGL J0623.1-4143SUMSS J062242-414357?åÒ£œÑɑ?ÈÀEÜI¡?ÔZ¸Æ\lÞ?ÈÀEÜI¡?æ—{1Ú?Ò7…ÊoÄ=?ÒÑÝÓ	œL?Ò7…ÊoÄ=?ÖÅJd°Ë?¼!T½Ó8™?äZͧþ›?¼!T½Ó8˜?æ©Ës\W?´™þJrÒ?Ò¬iGQþ?´™þJrÒ4FGL J0622.9+3326¿ä¦Áœ@"MŸ±áŽüÀ8k"ÌÐÿÀ;fr° Ĝ@VfXN ¢@D:Âs­? §?ä5bý?´8p)³®@KïIÏVë@azXᘌ¿ÑI
`EË¿Úölmçd(¿äÿ­õœ¿áWÂ~ë'¿éB=äg¿ã¶ô›»³AGNBCU3FGL J0622.9+3326B2 0619+33?ïö›5â!?J7
}
?RÈá";»·?J7
}
%?ïòtƒN§?q
ÄÀ¹²?[ãùb´f?q
ÄÀ¹·?ïWK?˜@¾i?ž>õ=–R?˜@¾i?ïÿîĘÕÊ>Þzr^Ú>á;g*64˜>Þzriu4FGL J0623.0-3010?ã÷ԑ_+&À2ëèPïÝÀ:Žf5¾þ®À<WoŠÑ€@sªZ1#ä@üCbU_®?Çy-¾T9?È´͆†?ÿ4i^hk#@	—49˜}¿ï©\ºëù¹?ïþ•œ´×
¿çýŠ¥
$¿æÜþ]¾w¿ë>ÝöÀ¼¿ïÿå(
eCAGNbcuPMN J0623-3010?ïôû˜??]s¡9"µ?WøÏł´?]s¡9"«?ïø]ÊãI?rk©öІ?N‹ÐÔrØ×?rk©öÐ…?îwà'.è?š¸ü`ÕSÉ?¨öí~'?š¸ü`ÕSÉ?ïÜÅ€Ëñ?b=Dí¦(±?qs?šò?b=Dí¦(±4FGL J0623.2+3044?ï`Õðƒú@ ¨½#žÀ9Ù©-‹TÀ<E¢Ë@ ¾!Š?üS€*\ÊÜ?Àµs>æð?Ä=ʗ"Z@'üÕ©@&ïjÜlÓ¿âDrØ
¿æBw©"É(¿àø]©ÿBk¿Îêq"'¿Ý`QyoW§¿ç®Žd•AGNbll3FGL J0623.3+3043GB6 J0623+3045?ïø)G÷Ðs?L0'Åê¹?OZà ¾:?L0'ÅêÅ?ïê!Àë'Å?†¦®ëz†>?eÞ?Ø;¾?†¦®ëz†=?ï¤á\ó?…ú¬>ûÔ?†Ç¨û»?…ú¬>ûÐ?ï¤s։´â?tpÌ)…t?†ã
]'ÇÃ?tpÌ)…u4FGL J0623.7-3348¿íÈô&¿ÉQÀ4[À6ãÀ9ìuk¼ç|À< 9€
@ Z¬Hóº@bê¾O[ˆ?¶Ô? Á†?ÆÌV»£…@ºk
F@ëc`w?ïeáÜ(Š¿Öæ€',À¿ääµ Þ¿ã²æ!1¨ï¿ë"Ÿ»Ì¿ïù)ÍAGNbcuPMN J0623-3350?ïÐ\Qóý?v'üõB2™?wÀQפ?v'üõB2š?ïøhÓÅ¡?k£"zÐ?N]ˆ°é~Æ?k£"zÑ?ëqçˆKk?©ŒùœVÆ?Â;¨aÞÒQ?©ŒùœVÇ?ïöñö'ø?AÅÖΛ?RøúB?AÅÖΧ4FGL J0623.9-5259¿æ¬ïHM'àÀ9[ѼrâÀ:è	¬Q,BÀ<£O•i‰1@yfÞ±PÅ@Á¶ža?Àd鎤s¿ ©Ü1ï'H?ãæ¹Ù«@K^ù	¿ê''Ò¬á?…pU0ð¿ä&½2%¿äO%‡N"¿Ò3f~¿á> AiõAGNbllMS 06225-5256?ï÷$¶–œƒ?KZ~̅m?Q¶'ÒÆù€?KZ~̅H?ïýGeû3?TvùãÜ*?5Ã|Ð&d®?TvùãÜ1?ïÜûñÓÝ2?tv »\·?q'g'?tv »\°?ïð"@$Â@?N&´t"j°?^÷¶{~¾?N&´t"j'4FGL J0624.2-2943?ÓÁzÓÀ2ƒ`¦3À;-Á>#Q>À<šnkîe¤@ g
Tý2p@2fâ(r?Æÿù_|è3?'îƒx<t?¸paö"@íW<ý·P¿Ô5k×ÌÛ¿ïÕrùà0?ëFúû´@å¿ãÚ­Ëų¿ê&ÏAò×?ÌJry\ãAGNbcu1RXS J062422.3-294449?ïë0'Øì"?`þw:b@?dÏm'Ý?`þw:b@"?ïý•XöPù?Pê%[i·?3U8Mx1¬?Pê%[i²?ïÿ&Þ7ý?Šá)]6¥Z?‹À6Hr	?Šá)]6¥^?ïìlvS¤?UÈÃæÔ6‰?c"à‰¬] ?UÈÃæÔ6'4FGL J0625.3+4439?ﹺS8@,Èdìé¢ÆÀ9p-ô/fÀ<-ëÎð"{@+'þKË@j0¥º9L?®Š°av|?©|ýÇ%C?úÔ:I§é¾@
8
û1¿Þi"$a¿ÛQìüíüÈ¿áÖ¸ÞÙ>Ë¿á&ƒÝo²@¿â¿Ð/WÜ`¿ãºû~ÿ—AGNbll3FGL J0625.2+4440GB6 J0625+4440?ïüÐÕò…¹?5P—Áö?9yPkÒ-?5P—Áâ?ïú<–Ÿü?a/s—u?G
§ñ€V?a/s—u?ïèÚtÏÔ?osLaoì?g%‹ë0,Â?osLaoì?ïá5A/Ø?[[¥·%?nʾÐ'ïO?[[¥·4FGL J0625.8-5441?ì¶8KS»À9o¿aª?À:5C•%À<VH˜F@Úäå@o–@HÅl?¿o"͊aî?¶šÇ—æd?óƒ
€òç@	¡hðÚH?Ë&`¼Ù9ÿæk%^¿ê«ᚺ+¿ãu"Ód—¿ïþŒÍÙ<G¿ïô€d{AGNfsrq3FGL J0626.0-5436PMN J0625-5438?ïþÇÀÚ4â?$ó­»DR?#ƒò\±Þ?$ó­»DQì?ïú%)—÷Ñ?`h"?%b?GkY  µ»?`h"?%bŽ?ïàÚø@çÞ?p?€ùèÎ?o%¿ ™?p?€ùèÉ?ïÛe¯Í*á?`ÈtBp¶æ?rM(jy?`ÈtBp¶è4FGL J0626.4-4259?@LýÕÀ6qgÛ±lÀ:gØp¤®À<rZؓªl@ =é[;e?ùXñ°C?ÑIÓގì?ÊGçµ±RH@'í]f¤@-æ–Íar?èM!*È+¿ä'%ߍš¿áŠJ;tÈ¿Òu.`µ*¿Ü4%áæåR¿éäóiï‡ãAGNbll3FGL J0626.6-42592MASS J06263670-4258059?ïý?Îzû(?3G@ÁTG?6Œ(&Æ[?3G@ÁT\?ïýÒ,0Ý(?Ip¶¸œt?1nžyÏ?Ip¶¸œ'?¡*s
?…ã^Gú×?‡W×µc=z?…ã^GúÝ?ïøv|õ¿^?;Ue)®ã?N&)‹Í?;Ue)®Ì4FGL J0626.4-1712?춁	áàäÀ*FhEZ}À:¹%8ž¬ÿÀ</½ÿªo«@<ä1˜Ss@<à[?Â¥ýÖ.
¿¡K×ÄÍyñ?àwU6":@bÀõ(5©¿Â$ޜ-Ä¿æb­¿keT¿ê'v¹Ã?²Ò<ççÛ¿ç+Zâ#Ì
¿áã+~3ÆAGNbll2MASS J06262650-1710467?ïì³Á~ý?]¹[E&?cLä>Ã?]¹[E%?ï÷W>@?oªìgÏR–?PåQƒÅV?oªìgÏR—?ïÀؼmþ?ƒ7Qˆ8´?ñ¡Éª?ƒ7Qˆ8°?ïæÎ`x"ÿ?XP=™9´ë?i1Ÿ‡Ýb?XP=™9´Û4FGL J0627.0-3529¿–ËÅÂU®À3ø2¹¯æÀ8êe˜ºÀ;ÚꃖøÕ@è7cnU?þM€†£Ð?¥I['Ý?'AÒiCæ?ìf¡t¯T@– 5T –¿¦áÃ\"31¿ßZžœ¿Ç¿à[Õì¿×Â"µí¿àŠEžoÂ0¿àæÂÂ1é1AGNrdg3FGL J0627.0-3529PKS 0625-35?ïü+tsª‰?7ÖIÀÛÓã?>¤\b«µ"?7ÖIÀÛÔ?ïüÂ]f"?Ul–ùyE?9ïÎöÝ?Ul–ùyA?ïé©×-ES?us%ÕZºô?fV(Òº­p?us%ÕZºä?ïé>Z6i?U$-f°Ž?fÁ¥éɖU?U$-f°"4FGL J0628.6+6900?ÔK/.³Ç"@75`A‰7LÀ:¶çºŽÜ§À<¯Tæb4@°´k½@j= ÿ:?ÀF¨0
_?¥0¼ê½µ?åAa)ÃÂ?üPåüéö¿Ç?›5ûåi¿ßN€2ÀG¿Ýߋ€Ò"w¿æîâ q¿àáÕ<ÝÖà¿å¢zH›zDAGNbcu3FGL J0630.3+6906GB6 J0629+6900?ïÜqUSË?jêì¿í?qøGUVé?jêì¿ð?ïõ	Ó©ü?iä{®nâ?UìX¬õ	?iä{®nâ?ï¨ÖõW"?"n‰ÊÀl—?…ÊB¿*?"n‰ÊÀl'?ïQ3 +uI?|ûÀ'òêf?•Ù‹ú'Vö?|ûÀ'òêd4FGL J0628.8-6250¿äfPxx'[À:vø½ì_9À9—Ú\ØHÀ<]õ£…«¦@Ûwy´!@ä̂úñ£?²ñLˆï¨D?¸¨xY­ñ?@GË $b¶@i}G(‰¿Ü¹­6/¿ã/¸ToÃÝ¿àÜßõÉp¿ãòžþˆ[¯¿â.•ßе¿ïÿîͨ"ßAGNbll3FGL J0629.0-6248PKS 0628-627?ïý»âîm!?+%"*û?2 茖ú*?+%"+?ïý­Iü?JÁ`âDX[?2"°x,?JÁ`âDXg?ïÇè0³º?~Yvò6ÁÈ?|çò¦"¬?~Yvò6ÁÐ?ïçUG4?T ´óª?hªå¸ËóÂ?T ´óª4FGL J0629.3-1959¿è Ž¿IÀ+U›=ÈKÀ8¦$'–GÖÀ;ŸñvÐ@ö@í®Š)@/L{ٕ2?¤þ€_G‰?²{婒‹@7b|×Â@¡ù5‹}!?îÿ5Ÿôým¿à;Ø»¿ã죗I]A¿âYÿ ^¯¹¿å•[|'˜Ë¿èK×nç>hAGNbll3FGL J0629.4-1959PKS 0627-199?ïþÆOa?%]^qˆ%?."ž›	îø?%]^qˆ%²?ïû­U'š†?Up1:è]Š?AJ©µ•å?Up1:è]‹?ïÇàpïD?{öéîìGè?|Lj8^;?{öéîìGâ?ïÿMŸg»?ÕV_ùZ@?_ln"?ÕV_ù["4FGL J0629.6+2435?ïâŒy$lÝ@ë—¦zSÀ:w,50"À<6¯A@ ,IõÂdi?þ§,yێ1?ÆÎ'€L–‡?ÊÜ >ú;Æ@Ó#þâÊ@`KZS3¿ìõcߣi&?ïû0Ãj¦?°\ڗe¸¿Ü¨
»)Œ@¿å­Œ?¾ÜÊ¿åÁЄè1­AGNbcuGB6 J0629+2437?ïòú«Ã½Å?[†¯®—?Z
¨x"tÊ?[†¯®—?ï×ÓuWîK?'ó·àØN[?tETÚH?'ó·àØN\?ïÈÿ¢?–¦¤ÜÒ°?œüÀ¿G?–¦¤ÜÒ®?ïù¦ª»?‡i}"^?œ`Ë*¨?‡i}"_4FGL J0630.2+3228?èTÊZ)Q¿@$4D‡BÀ;Mä·¥[À<}Pǘ°@ ÿ€Êì?ÿ°g܈+³?ÏMyÛc='?¶"¾ì†?é\>ŸÍæ@Xg‰Q"¿âÄõ"+y?î°LÎå«Á?æÿN)X¾Þ¿èY¹Å¿à9™m$?—àèžË˜ÖAGNbcuNVSS J063010+322608?ïöZ¸I³?[¬{{ð?SJm蚋?[¬{{õ?ïôË#d™í?s¢âŸ<¹v?Vi¹6Ì$M?s¢âŸ<¹v?̠;?‡ۂó?ŠÌ×ñá?‡ۂ÷?ï­¾XÌð?uÀ4çϬ%?"{©ÌÃð?uÀ4çϬ&4FGL J0630.9-2406?ïS5b=_çÀ-ý˜ZÕ8¬À7Å™m#ðÀ;'>[…b@â³¹€iÈ?úw¥ôïp?›h´§ð}	?·³ìŸ@©"þ×áÔ@²¤­sì? Õú¿É¾¹ä'¼0¿Øtߚ¯Ä¿×{Ì¿‹Æ¿Û½ûx±Â…¿â™
'¡/AGNbll3FGL J0630.9-2406TXS 0628-240?ïö±¸ ²‹?QÚIæVËQ?RœŽ¾šê?QÚIæVËP?ïºGðC?–aI›¨0?nþo9Ò?–aI›¨0?ïn<Ûa3?':''X?'8dŸÓل?':''X?îÖãm'V?'³ƒÊ`—?¢'Î-Š«?'³ƒÊ`—4FGL J0631.1+2020¿ãäр>…"@gŒSâÖÀ9kÛq«>À;—Ìe÷@@غÿñ@á">¿?Áݚzj)j?Êâë݉2™@'%ùŽÌ·@ð{Dü¿é7FBÐ_¿Íñ<†C&¿á§˜úà¿åàZéZ¢
¿çÀØ!ê‹z¿ïü-ãhÅAGNbcu3FGL J0631.2+2019TXS 0628+203?ï@<üº?;?–•'ÂT?—ø`h¸©?–•'ÂT?ïîß1}d?…íÝózX?a ΂ùœ£?…íÝózX?ëà	m³X¯?©u{Mð>?ÀÚI2G?©u{Mð>?ïàfósõ€?]ð*fÞ¿¼?o™Œ
y?]ð*fÞ¿º4FGL J0632.0-1032?î³Ý©¦àÀ"ÞÁÁÖÐÀ9¢sۍZÀ;¶^	}@‹0k,ɸ@æ*C hÁ?¿Ø×á—?¼ô
ÔDe`?ú̺=~Ð?ùqï-Iå¿áí¾´Ü?¿áđ?h¿âJ/-êôÖ¿çaZž:Ø¿ì‰OŸz"¿ÚCTþßïiAGNbcuTXS 0629-105?íäì`ø.?°'	L
3?°Øœø>m?°'	L
3?íEÕ*½M;?Á
MÚY"Ø?µÑVª–2?Á
MÚY"Ø?ëµo!Õ?¨€¯';‹-?Á*Cx«ï¹?¨€¯';‹-?æÛòÄ£?µ"þÄy?ÒIæÔv¹?µ"þÄz4FGL J0633.4-2222?×OÂ]mˆBÀ+‰
Z[–)À:.MeÀ;ó£BÇ‰@Sϊí.@##—´½?ÁhÞ»·§?Ҋ¸?Ìô@"]Ä×5@f§€âéo¿åÛ1´­ò¿Ù§MKã-a¿æE'`À48¿êðÚ'ÿ"Š¿êŽ€á¼Èô¿ïÿ[ËñrAGNfsrqPMN J0633-2223?ï‰I¥æX¢?‰®Ì{?­–†i׿?‰®Ì{?ïûÔaº?Wæ®sqÚw?@¯¢y«g?Wæ®sqÚp?êO"KmÓ	?©ÿþ5^¸µ?ÆÃvÒH³Þ?©ÿþ5^¸µ?ïôx\PR2?Fö™0oñ?WG_[«?Fö™0oç4FGL J0634.9-2335?ï݀çSK$À+ë[³"ý*À9ŸŸ¡—[À;öюÓlú@b
#Ôñ^@Ì{n5h?¹²áØçQ?´Eæêk?ø"Ñ ¤<@ö"‹ë[-?´ãAƒXµ¿çň4íH¿ç>—"ƒ¿çÖ!ªt³¿ïÿŝƒ‰¿Î‡¾ bAGNfsrq3FGL J0634.7-2334PMN J0634-2335?ïýœ'ü^?8Àì@?3ûp,?8Àì?ïð¡Ò?xø¬'˳?^½ÇéàYÅ?xø¬'˵?ï´Êz¤.?Œøn*?'ÍaVþ4ž?Œøn*?ï¢âCêî«?sÛ·N¸ª×?‡GoDUM?sÛ·N¸ªÕ4FGL J0635.6-7518¿ëÅM†ò6IÀ;+Ë£!hÀ9"tnfæÀ<!™í|o½@ûPO£¬B@…×ÙôÓ?§zGÞÁp?ïé:g}?Ýò@úœñ@kº%€B0¿Ýﯛ
·ú¿ä†l@E‡¿égÿBÀÅ¿é»Âîýy=¿è;å¿ê¿á["{L§xAGNfsrq3FGL J0635.7-7517PKS 0637-75?ïÿ…99h?
?{†è?±±¥ÿ9Ø?
?{†9?ïþ`‰=Ü?OÙo×yC?)÷l#Æ2"?OÙo×y.?ïÕò?ôn?v	pŒ]s?uà@ȗ?v	pŒ]u?ïÿú
¦¸>Š"âß:9>ÇÉeÒ!>Š"âß-¸4FGL J0636.5+7138?Çó`Öºäë@8~´Øº@ÙÀ::ªù›À<[@ےbn@Eˆy`¿@¨[ü€¿?¹há?öe"?´Õ³{B¤?÷1^µ—ý@àl
ë?ïë!äVV¿ç5A•Ì…¿æwô˜Ã°Ä¿æ.ÕÀç;c¿èï9©nù³¿ï߄¬°AGNbcu2FGL J0633.8+7132GB6 J0636+7138?ïü؉ú1x?0dï®Áè?9;°.t?-?0dï®Â?ïý'¤¢ß?QP¹à³å?3jÚéX?QP¹à³÷?ïáp˼X?kkåÁy¹2?n4ìC§J?kkåÁy¹6?ïþÈ
2Tã?$üAýh?#,Ú±Ín?$üAý4FGL J0637.4-3537?èámzPUgÀ2	t²GÀ:ž—•}À<xŠ]¼t@tècV;¡@
Ù©T"?ÆÀéª(2#?ÃuG?Y²#?øB*aÓY¯@2Ot\sH?ïÿôÂ_5›¿Û‹4œ>ån¿ß<߆d¿ç&zü	¿ßԜåS\¿ïÿŽ‹HÿAGNbcuWISE J063746.40-353648.3?ïçhù
´'?hf•¬:üË?h—õKom?hf•¬:üË?ïØ-™"ûÁ?"~þ2˾›?sé36Ï?"~þ2˾œ?ï1ø"&ӛ?'FY}ß?™Àï{%Œ?'FY}ß?ïÒÅr?ƒç[äNkÿ?œ§]½'°?ƒç[äNkÿ4FGL J0638.2+6020¿Ûl›Í{o5@5Æ՝Uæ¼À:Þ%‰ýDdÀ<'û_‡O@&cõÑb@ÿJ˜ª†Q?Ê"кm#Å?Íf¬¸ZO@ŒþùoÃ@hgÝ	¿ìÿº_⾧?ïû';&F¼¿å½xÁ‡Ê9¿æü»bJš¿ïöÃÁ5iï?Ä1ˆ8HEêAGNbcuGB6 J0638+6016?ï[ËŠ{Ð?šÒ¼óæd§?"ÆŽ°†)?šÒ¼óæd§?î.üÇýƒÞ?Á©¿ÿµ"?­3€'Â?Á©¿ÿµ"?í:ÏrW?£N÷Öaã?¶/لo…@?£N÷Öaâ?îYêÓ$h?—Óo(#g¶?ªaRÍ¿Iu?—Óo(#g´4FGL J0638.6+7320¿ïûÍ?1@9ºùe²À:ó˜éprÀ<Mš#×v@!T‡ÁªÛ@-»Å=ŒS?¹¶2‡?xmّ2ö?»£Õݗ E@•§ˆo¥ª¿ã€¹ÎÃG¿ç¡L'HD¿ë¾Àdß}©¿é£"î^íÌ¿î6±•+v¿ï«WÂ3Á£AGNfsrq3FGL J0638.6+7324S5 0633+73?ïþw­ªÂ†?1Z£ê¸!+?(…%S×® ?1Z£ê¸ á?ïýl)љ?X¶g:y?4Ÿö±s<Ð?X¶g:s?ïÍBÑÛWÜ?|–õlí2?y^—T"?|–õlí3?ïü´$"ôÜ?0ÿ8R!?:^Û`Y"Ž?0ÿ8R ü4FGL J0638.7+2753¿Ú%§TK
ä@##_€™À;K§*{ԍÀ<œLŠN@!Y¹óA‰?ûø=^/`@?Ñ&ö¶|?–;֚ÖÛ?õ~…&E'?ôkڔ5¬Š¿ïÿï¤h)µ?è%¿âÙ~Œ?ï÷€Õ}uw¿åR÷Ù.Û¿ã×ýsº?Ë‹i*;AGNbcuRX J0638.6+2751?ïõ|)z¢¿?Y'ªŽ,ä?U­
ºƒ&?Y'ªŽ,ã?ïÌé'ÐÄ?¸{I73Ž?œFbÛç"?¸{I73Ž?ïsË­¨0 ?‰9·è,ÔÔ?'†ŠJùû÷?‰9·è,ÔÛ?ì³½Až£?¨eAH4?ºgbó
ø?¨eAH44FGL J0638.7+5658?½Ê!|e@4ÓDZ¢äÀ;
X;*xzÀ<›b§K3@¡)œ±|@¿¤Ùš;?ΐ¸‰ôµõ?ӜqeHO@‹"˜€"æ@¬@?¶#h?ïî¤!²Ø¿æUïÝëÙ¿é(ÒxÞ¿äœ¦°)¿ïþ–¾ßú¿ìÝE ž³AGNbcu3FGL J0638.4+5704GB6 J0638+5701?ïõîõ4R?Zsñڀҡ?T#ЗZ?ZsñڀҜ?ïD‡"@cç?®lvûÕÝ?—o
wó'û?®lvûÕÞ?îꦴ¦
?"oý̜?¡U"µžß_?"oý̜?ï/ù¹Èù?€Þíôñ?šÈÆüàõ?€Þíôð4FGL J0639.6+3503¿ä^à[ä£@)í¢Pø@À:Yã|;ºÁÀ<(ѧýàk@2Pó€Ý@9{ßto>?¿0öíݓ™¿ª¢ÒÛãÐ?ëu'Ìö¾@\T‹GœL¿á˜
þEjÿå¹ÝaD"ƒ¿ì/s‹¿ÓÄ{ÚìË¿ìÈ÷?½X¿Ä	´Ÿ.ƒ÷AGNbcuB2 0635+35?ïÙ¤V¹?r»2^0Ns?s-ðqT£–?r»2^0Ns?ïÏ­Ô?0X?¡5·½	2Þ?x)àgÔ%?¡5·½	2ß?ïƒ	dD½?Œ«ë?€?=»¦îÐj?Œ«ë?€ ?ïä}ڜ›¼?`Je¹Ùùô?k'%cdD¾?`Je¹Ùùø4FGL J0640.0-1253¿ï•À› 4À ¤€¥¬ÍSÀ9é/bÄwÀ;õ­§m—³@""†ÖHv'?ùÜسŠÜg?»~b MÓ?¢6,"9Ø`?åÛb'Ő?ù×E÷†	¿éx¶Ë¿åªy»­Á¿àY!95«³¿Î¹©™ìУ¿ØÃd£î‡2¿¶@¼ž+y«AGNbll3FGL J0640.0-1252TXS 0637-128?ïún8UáQ?A‡§{±ô?FG¨zº|?A‡§{±ï?ïîÌdNO?"f þiŒ?a3›±ì±(?"f þiŒ?ï´Ë"ëÃ?€š$+Ú?'Í<Û?€š$+Û?ï(Tm?²J?Žèá3Oõ?šõrX	¶ß?Žèá3Oö4FGL J0640.8+2432?ÒՉ±+ÑK@!~O3Cú+À; C÷¦•+À<r2ËŸ@!^Î¥?=?÷"]wª[‰?πl÷м?ׇS±Wü@@ÅEÅ@Ìÿ¹^0¿ïþ›A9†?ïÿöµš?d-o¶•h?ȯD;CM¿Ü\O™-
¿í1}‡ AGNbcuRGB J0640+245B?ïû'JÌNÓ?@§¢±Øø?AöÔÎĸ•?@§¢±Øø?ïê)sð,Á?";
Äü§°?e֌Ó@?";
Äü§®?ïjÜSÝѐ?÷PäÚæw?'¤u"EÎ'?÷PäÚæv?ïÆ+•ª¯?m²!'"½?|ê5s*¨ˆ?m²!'"½4FGL J0641.7-0320?Ø?nùBf,À
oZÎÀ8mô¡',•À;%ºÜ	€²@Îü<Ñí@nòÇ2Y?°—Uq¡'ò?Åß_vˆš@L{‰
Z\@ƒs¢¹ÿ¿ÑyÁ¢w8Ç¿ä,0àrœ¿çG–,&Ïx¿ëymª'†¿ïy?n)ÿ¿ïû!sîfAGNFSRQ3FGL J0641.8-0319PMN J0641-0320?ïõ}A'-?SqAm7?U}Öû¦Æ?SqAm7…?ïø_¾Ÿ?vëŸç˜®?O'ƒ‰ƒã?vëŸç˜°?î>²ÿÀ?¡#~·=
?¯OŒÐ?¡#~·=
?ïóTY¿£?IËL'ÔÅ?YWL€¹ò'?IËL'ÔÅ4FGL J0643.2-5356?ê-ñȂÀ6É/Ÿ¾wÀ:m÷hÉ™À<qދ;2@ÊkÃr†@"NÿA"?½>™~ýÈ)?'I©¹™¶—?ÓÿZS2¬û@\r˜£ÐT¿ã[m¯0Ô¿ãr2aüõ4¿ã£ð4°áµ¿äžh5s¿ë#î¼á>¿ïÿ÷1$e:AGNbcu3FGL J0643.4-5358PMN J0643-5358?ïþƒ`…D
?%uÁ̓û~?'É÷«¿i¡?%uÁ̓ü?ïþ£	ï÷K?E'1%_h?%Ïa‹-­?E'1%_h?ïÈÝíÒK?ùþ§iÓ?{'	Ú7ð?ùþ§iÖ?ïþöüg?«þ
;? 7™'Ì?«þ
ê4FGL J0643.3+0857¿ï•y:²À@Jf:Ç|+À8Eöx—ÁRÀ;w…@˜Cz~ l@ê#ÚЛŽ?ªeŒÄ'?Æ¡°êC*L@g:6\³_@žS;¿Õd¾{PX]¿à¤¥0¦ù¿çPáïɧ¿èó­aL¡¿ëlb©Ã]¿ïÿ†}³	,AGNfsrq3FGL J0643.2+0859PMN J0643+0857?ï©VÐNoX?‡OÖI§?…ªKìd*;?‡OÖI©?ï}!'óù?©
±IT?[ßíÁ€ú?©
±IT?ì¡.뷆
?¨#µNCX?ºöˆ¢CÏ´?¨#µNCZ?ïÉÊøŠ?mn\"ü?{t}ƒ»ž?mn\"ü4FGL J0644.4-6712?Þê'	B¶°À9‡ºùe²À8½CwN7À;̾&@Ü@œrêƒA@K²™ß:?¥ìAº¾
?¶ïôAðe@ì-BXj$@¾&-f?¥?Ù:!¹ä¿Ûn¤éb/¿âV<»È¿á½4ßݵ¿æTd ;ë¿í»Šàn?NAGNfsrq3FGL J0644.3-6713PKS 0644-671?ïývpW?1'.Y­?7$Kô}D¯?1'.Y­?ïû	¦XW?`†ÂÿvO?C·Ùfž ï?`†ÂÿvR?ïªP¸…5?‰*X©¨ÿ?…kÑ؞²ÿ?‰*X©¨ÿ?ïÿêZß>à+uþì}>åæ¥ ê³ª>à+uþì4FGL J0644.6+6039¿à \›WT÷@6ÔÇm{À:_þKÊÙ®À<'©1½n@'²'
@a× åÂ?»c òÏý?–ÇùB:{ì?à<í'hr°@Z]ÿ—¸?ïøC""~¿êxdàTi¿áZÕ¤ãc¿×ðŒma,¿àШ# 9¿ãzˆ\ZsêAGNbll3FGL J0644.6+6035NVSS J064435+603849?ïþ™I'xz?(ܐ,˜¨?&kmˆxV€?(ܐ,˜o?ïþd3º ±?EDñÅDÊ¡?)¼ÄUõ8?EDñÅDÊ­?ïú‰'¯D?]4áAPK«?GÑÙ¹Bï?]4áAPKÌ?ïüîðJ)Ã?%L"˜¾x?8ˆ}®±Ü?%L"˜¾x4FGL J0644.6-2853?î«£KGÜÒÀ,&o"5ÒJÀ:Í»DLÊÀ<iŽ2]J^@ Ó ñ§£?ùdM‡rO©?ʈBZ¨m?ҁþÝÁ×@	bçcQ0@
hs[í¿ïÿ› 'V‡?ïó¯ûî|?ÀEýz¿ŽÌ¿Û'@5пÏ	IÕ·4¿æ²d ï&AGNbcu3FGL J0644.6-2853NVSS J064443-285116?ïÐïï˜;?y€Ã¹I¤š?wð3â|?y€Ã¹I¤›?ïÛÁŸ+­é?n\mçT?r0j)r?n\mçT?î	–È›—?¢t¹Ômëù?¯f"vN"?¢t¹Ômëù?ïuo)T?‹`d,¼†ò?ŸRÕ~?‹`d,¼†ñ4FGL J0646.7-3913¿í›_Ç»ŽÀ1›ÜY1Ê}À:JiýʛšÀ<HÄdH~õ@–ìËÅ»¶@wdã¯ga?Ä:DŸlAr?¯'ªa4oÁ?ãzksù@	‹–ßU§¿â§´«å¿ç¼¯ŒwG¿ìc1" Õ¿è«k…L¿ïþrÎ\¿é¡–R½<6AGNfsrq3FGL J0645.9-3914PKS 0644-390?ïÿ¹¢X*N?pÆÓrb?—iõlõ?pÆÓqÁ?ïözŽ§]O?sCuv¹…-?S
â±Eaœ?sCuv¹….?ïÙµe‹?têQ€b–˜?s%|M:},?têQ€b–™?ïôƒâ2{?I[ïçßFý?Vø;›É	G?I[ïçßFã4FGL J0647.0-5138¿îi¸q´"À5—Ø'sâPÀ;•YÀ<¥øZQ
@!CŽqwÛ?ú7ZYè©¢?ÏÌt7_gÅ?Âm9©Äßî?óTsۍ@­Ô€Jh.¿çX-ˆÏFû?ï‰ü¾, ¿åþ‹#¼H?Ò$Œý)¿ä6Ÿ™Û¿ÐÛPž(­AGNbcu3FGL J0647.0-51341ES 0646-515?ïÿ9|0?‹×Ú@Ï?ÐyýnÑ?‹×ÚA?ïþ7B@à]?McúÂ_?,‹Ûñú(?McúÂU?ïé5_¦ÍÀ?p|o9Fa?fÊ Y2>Ñ?p|o9Fd?ïø;þñí?B'ÑuX‡N?O÷8M?B'ÑuX‡/4FGL J0647.7-4418¿æ^
'zÀ33sâOëÑÀ:Ãf½ÌÀ<"ERðgÝ@Òÿ+ní@='¯š?È\S}€‰R?ËW\È­ÙB@·kÜÇì"@äNs«s?äšF½©™A¿ÜùÀGƒL¿ä¢­>'¿×˜Wš¿ëé¡éÛÑ¿ïÿý{ÁA~AGNbcu3FGL J0647.1-4415SUMSS J064744-441946?îÐ/ÂO¼Æ?¡¼Þ¼™ù?¢ýÛ3¤?¡¼Þ¼™ù?ïÀkƋ¡ç?›lìK·C?ʺ/¯?›lìK·D?ì÷Êa˜¥?¥¿bÚõ7?¸A¬ó?"Ô?¥¿bÚõ9?î(¹7Ó?‹ó•Ð©*>?§
tlƒÆÔ?‹ó•Ð©*>4FGL J0647.7-6058?èvÇ¢PÀ7ï´_½ŒÀ9ÆöÞN«À<R«ÿÍ«@ g-Å`@Wç^j?³(¤9Ù?¥ÐKÉt?ñà^åh¥@ו9?Â(mÀοæ8éU™¿ænÖâÐDQ¿ãIŠ"-Qr¿í7!ŸŒø¡¿ÑH¹­5WÑAGNbll3FGL J0647.6-6058PMN J0647-6058?ïü¤Ö‹Ë?2Œt«àí?:ÙK§)§'?2Œt«àð?ïþ4®Š u?Mq~~K?,µ]ø±ù?Mq~~X?ïåŠÚO?m"w]Òw?jùu%°ïž?m"w]Ò{?ïþÂÙ°tH?|ëýkZ?#Òdø»š²?|ëýku4FGL J0647.8+4527?ã8ôœÐTÅ@2_–لÀ9ÏÒ␃pÀ<žßS¸@"mðÉVK@/»õäô?»ïj0 [Ö?º®?-÷?øäӛ'@¿ü¯¾¿W…ï(þb,¿åýÞó?þ¿ë4úqK¿éªBÿY¿áÑCõ"Vl¿ïÿçáüúAGNbcuB3 0644+454?ï¿>(QPß?'ºÒ("I?€0uë«È?'ºÒ("I?í9ÿC?À(Eʃ‡©?³0çd?À(Eʃ‡©?îÞ¶§Ì˜? W"{MÙ?¯•ƒ6k? W"{MÖ?î>wú¾?˜%×膰?¬€^"+?˜%×膱4FGL J0648.0-3045¿Éˆ¶Ãeð3À,M‰ÎJ{NÀ9^íÌ ÕÀ;öJ…_Oò@/"⥧@tÁrüw?ªc;
Ȭ?À¢½¯£q@lN¡MÃ@.y¥ˆe??Û¡Ñ@ÏÓè¿àXR§lÀó¿èl3/u¿ç2,ئã¿çØì`¿ïÿî' ÇAGNfsrq3FGL J0648.1-3045PKS 0646-306?ïýhـ!ø?5]nºtâ?4¹3þð??5]nºtð?ïúъµI3?\0ò>_H?D¹Õ*Û3{?\0ò>_E?ï¤7l
ìà?'
Eð«Ä?†ò$ü"È|?'
Eð«Ä?ïþ䉋]?¡¹´¼ð?!·gNZ0_?¡¹´¼F4FGL J0648.1+1605¿îì˜úP@9GüÀ:îÓr&ŽÀ<cp'Iü@!Cö6D5?ûËh´€?Ë5ª†ÑÀÒ?ÃKé¸jë?÷!iÝl@š£Š3J/?æÌ0$ŠùÄ¿ïžQYŽç?ïþ"Õ½6W¿à•NEÞ0¢¿ç榒¦`¿	ã‡AGNbcu3FGL J0648.1+16061RXS J064814.1+160708?ïø*âÖ8?J!ÿ°d?O—Tt§N?J!ÿ°]?ïôw:Sʨ?x §Ë?W‹Xj®!?x §Ë?ïÊÄk4l¢?}•ÜÕwñº?zÊeɯO?}•ÜÕwñµ?ïÖÂø·+?€­bÇ܈?ŒŠOAÒ5}?€­bÇ܄4FGL J0648.2+1745¿Õ
ÊJ6~í@MþûôÅÀ:ð‰¹QÅÅÀ<]vâµl^@ ݁ñ\N5@¼râv?Á=èƒažÖ¿´Ã$¹ô?òÛ>µGu
@1ùeÜþž?luS¿ç
'àÂÍð¿çeþj~¤¿ÛA"YÁg¿àyVbã$'¿å®éŒöóèAGNbcu3FGL J0647.8+1751GB6 J0648+1749?ïö!š]µ#?KCÒö Ì?S¼ËD•º7?KCÒö ¸?ïì˜ÐÁ8.?€ºŽ'½³µ?cg/>ÇÒX?€ºŽ'½³µ?ïðÞǀÄc?i¸'å-fJ?^Bpþw9‡?i¸'å-fC?ï›ÿˆÚQ©?räeÄf"?‰Ék•ï?räeÄf"4FGL J0648.4-1743¿åNÓ¿xíÀ!=‡rO¨µÀ8:êh¿;À;7SåZbL@ªšhÌr4@í"Zm3à?¥Ñl»?Ào>|<'@ãxt†@*‰
tx¿×Uˆà%¿â×nc¨¿åîŸ	›	¿æîQ Ü"¿ë1ÓíR~R¿æ"% ËÒ|AGNfsrq3FGL J0648.8-1740TXS 0646-176?ïîU{ƒÈ?^ýo@èËÑ?aþª"|6Ï?^ýo@èËÌ?ïîâLU<â?ŒóÆõ'œî?a³ªÃå?ŒóÆõ'œë?ïPjW«S?'€¸Ï¡Gž?•òµʕ¨?'€¸Ï¡G›?ïÿ7Y6? f€·1'?9Ù?É? f€·1&4FGL J0648.4-6941¿èbIW¼aÀ9'h›Œ¹À;×5>¦À<üF€íÑ)@!M˜.‹?ü°åEi–?Óñž"S"?ÂwOWV(+?òeR…?ù(Øç7\8¿ïÑ£Ì"'â?ÊUÆ[ªq?ïՄ̂úò¿å']džg¿·ò'ÿNTL¿âù¡A-ǹAGNbcu1RXS J064850.3-694519?ïúƒQϹ?Kjýý¸Ð?Gµò¸Áe?Kjýý¸´?ïü"ÎW¥?YjL"­?;ُMBÍK?YjL"µ?辶'ö?ƒ2¥J#g®?…–_O;Ÿ?ƒ2¥J#g°?ïÉ{©Uã?qy©ޒJ?{B+|U
 ?qy©ޒJ4FGL J0648.7+1516¿ßz0H9šß@KÆ!·à¬À8Û
LŠNÀ;ž¡[.ú¿@!³R)˜?ú¿gJ¹?¨Ã¤¯ø*Ê?¡œbY¯ý?÷¢™Øƒº4@ ΁­¿–?íók›Æp?¯H\æ
¿ÙςŸ,*«¿Ñâ"~ea¿ÚfÝD>He¿ÚI"ÇȁAGNbll3FGL J0648.8+1516RX J0648.7+1516?ïû¢EÍS?<ÒϺ9U?Avèʳ°?<ÒϺ9z?ïõoǾè?o~ã¨Ó?U pƒÒ/©?o~ã¨ÓŽû?ïƲ
øÖ?™]B¿0?|¦úƒ"üø?™]B¿-?ïØ~N_M?apßRÙVü?sÀØÐ~Y+?apßRÙVù4FGL J0649.3+2230¿åCLâJ7è@#<yÔØ4	À;&oþDÀ<~+qÒ
@ ×´?˜?þ·.ÕÖ`Ê?É¡Ä
†k¿?œ?÷Wó?Ì6sCš@8Jaοï{KeY -?ïþ"åÞÊ¿Ýû'¾Šêª¿á$"…|+¿ç…Õ"ܤ¿ÉýC¸¨AGNbcuGB6 J0649+2228?ïý‰-mz?@¶¦û'R2?3¶"—Œ3[?@¶¦û'RG?ïúØé¬Do?g±*ðN?DœYNîA$?g±*ðF?ïظ}Ч?w±õ"¶Ý?s£Á¬?É?w±õ"¶×?ïèsEþÜ?X⸅Ã?gŒºê"˜?X⸅Ã4FGL J0649.5-3139¿í¿ïYpe£À,k-M@$³À9þˆˆ˜ÀÀ<!V˜"	]@!«ÝˆÜ²ô?÷½w$#Ë·?Á=wš@]"?Ĩԟÿå(@©)Äõg÷@	«èCZH¿ç¼ dŽõÒ¿éÛiQ;¿ß[™C]wÕ¿·ùl'ûDÚ¿×ÙÖà÷Ò	¿Õ^ŠD<
AGNbll3FGL J0649.6-3138NVSS J064933-313917?ïýú>‰‰?1x9\cÊ?7h.³³|?1x9\cæ?ïû?RûÎF?hTýÏý+?C´Æçr?hTýÏý,?ï¯ÞŸàª?ƒŠÁš"K[?"˜Ռ?ƒŠÁš"KX?ïòóMá3?NbxF£C?Zd<śS?NbxF£44FGL J0650.2-1636?¸yQD†VÀî軶$À9"†AΩÀ;s•}@'/bn4;@¿~/°È?´…¢ì©Œ?¨›'Ÿgu?ò=ÂÙ.@
ï+E((=?ïèsAI¿à?Ä UàÝ¿éAΡ¹"̿塏Òpz¼¿ìÁr%·¿àÐ%FáeáAGNbcu3FGL J0650.4-1636PKS 0648-16?ïîÇ[1š`?b¶)keŽ?a8¤Îe >?b¶)ke‹?ïý51Lö;?X«p½ˆp
?6Vu˜N?X«p½ˆp?ïE$›€Àˆ?d¹æèª?—[lçï?d¹æè¥?ï؅þ—ö4?a£ê¸s0$?s½´æ›?a£ê¸s0&4FGL J0650.5-2851?ïCóÑ	¥3À)ÌE˼+•À:³D…klÀ<7äæŸê@¨Ïqí®@¯äë8?Ïœí¡ƒÚ?ÙX«þ +ï@$ÚZT	m@
™á*Qã"¿Î) zb¿æ}ÿ	_û¿è@›f"sÈ¿åýŒBn¦¿ïüA&PÍ¿ðAGNbcuPMN J0650-2849?ïúîCzÖ6?X@ñIÙ.?DFò§$¤?X@ñIÙ#?0¶=?¾+rÓN
]?¥ï‡œôœ;?¾+rÓN
]?îagx‰‰ô?›Óî0{›ñ?©éˆwg`Æ?›Óî0{›õ?îïÜÈ¡±Æ?‰°H¢¢ñ?¡3uäã ?‰°H¢¢ñ4FGL J0650.7+2503¿ËÍXŠñÃ@&áõ±ÈÀ7ËUúÞXÀ;$ö%‹«@U)[™ñ?úãEš>H?›QZ™1G~?Hõ<WŸ#@m|²F@~Ÿvþ9¿"Ô#ƒ<àÜ¿È"HJ¸á¿Ûúœ~Pg÷¿Ô'")Dó¿ÞÇýM´¿ÈJì¢ÖWAGNbll3FGL J0650.7+25031ES 0647+250?ïý;¬kå?1±õ0¶?6"œ ×¾?1±õ0˜?ïõ>ªï:?wÌa.¹?UႪ!Ž¹?wÌa.·?ï̈B˜ÊR?•ÞsØF"?y»Þ³š×'?•ÞsØF?ïÿŸ®æÔ>ÿ´vDJs?FJàÀ&>ÿ´vDK‡4FGL J0651.0+4013?ïÿÿ£º@1Å!Ý À9ÖâӟNåÀ<Q¹¾Ó@J
ÒüfÃ@?¦›à›·?µc¢áy­?­âDc\œ?öf
{ÅÕ@ë÷/ü¿ÞÎAìßg¿à>ÌÄiQ¿à1ZJÏ1+¿àõ·§¡š¿â¡5íËJ¿çÒtvÊa¹AGNbcu3FGL J0651.3+4014RX J0651.0+4013?ïÛ¯¬?­ZÖô+?e?r()÷8x??­ZÖô+?e?ïõÌ[o?¹?pmÍ©Õb?TgI!€'y?pmÍ©Õ_?ïԄ	'?~ó¿'°º?u½À{w·?~ó¿'°±?ï®z–Ú?oêQÿ`Ð?"aZzÉz?oêQÿ`Ð4FGL J0651.4+6525?é%¡X+û)@8ñ"<:CÀ:Zys‰d˜À<²®{¨íÊ@©µß†?þ±fYÑ,®?¿S>ìNó-?Ãb;ÉÚª@qÕ"äF@CP³¡­¿Ý
™E彿ãvõÊò×ù¿×L*ZÇvͿڝDÿŽk¿é
jKÎ4¬¿ïÈ<¿2ÛAGNbcu3FGL J0650.9+6524NVSS J065125+652458?­j3n?…eTŸÝ?‡T¥s$`?…eTŸÝ?ïï%y+±T?wXõ˜õm[?`چÔN­U?wXõ˜õm\?ï@Eåƒ?'‹9¯÷‹?—÷C]¼Ï³?'‹9¯÷Š?ïêpÓ¤?"jw˓2?œ"±ìE‹'?"jw˓14FGL J0651.5+7956¿äªj™Þ~@:®ÿ:Þ"`À;/Nbc¢gÀ<šz¿ÖD@ÌvŒyK@¶ÌD琝?À0D
û¿Äà7bÂÂÞ@¿*?nªÙ?ñÕ;0W·¿ì/AT©P¿És—ý7MÊ¿àQ½e¿ê˜YþyC¿Æ)£L¿ðAGNbcuWN B0643.2+7959?ïvöšfI6?¢a8ÞùG?'!,³6ÙN?¢a8ÞùG?䓐³Ú?Ô¥-‡Dc?ÖØޙÖKà?Ô¥-‡Dc?éš};^¥Æ?°n]݊\?ɖ…hé?°n]݊\?äœ'"Ñç?ďÙR÷¿?ÖDZº\1Á?ďÙR÷¿4FGL J0652.1-4813?îýŠÍY×ÏÀ3ÃäÿÉy[À;	¼AdNÀ<³""Æ@ 4'éª?þiÀ=rQV?ÎÜ垪Ð?Àÿ±%§Yv?ñð*Ÿæ»@Z²~?ï'usI£¸¿égý	«zm¿Þ?M]Uñy¿áïç"7Ý¿ßPcÛÅ¿ãΰœë]²AGNbcu3FGL J0652.0-48081RXS J065201.0-480858?ïþLé.~È?)Ý&Y^'?+1mrº?)Ý&Y^p?ïûѧŠÞ?d¿lUQ:?@¹a׀"f?d¿lUQ:?ïíîîtH?jb÷$
¡?b€‹¸5?jb÷$
 ?ïàtÕÒÐ?ZñÕ="?o‹*à-0|?ZñÕ=~4FGL J0652.5+1932?çÁTœGÔ¦@"	j­À:€ÈlüÀ<&D‰œÌT@jßÃ@zÓ}Àõÿ?פ˜Æ5?ߊë¡#P½@¡~4¹E1@ñ'1ó9?ïû	öùÇ?ĐK<>u¿âÛYWŠ¿ë¶¹ÐpÆ<¿ïւäY±¿ïÿ§ëkôEAGNbcuMG2 J065230+1934?å1u>`2•?ÍàýU&'s?՝ƒ?šÖ?ÍàýU&'s?àaÐzdgÙ?ÓXœcy?ß<_70N?ÓXœcy?ã«ÆFKwÙ?¶ò×釒j?بssiM?¶ò×釒i?ߦÜiì:?´ËoÇ¯?à,÷'Ë	ã?´ËoÇ¯4FGL J0653.6+1636¿íÀd]á~T@Û2‹m†ìÀ:(°ÿèÀ<7ÚH¶R7@–¼f@kÈ:–ÔÃ?¼= IŒ¿5óT|'Q@äO¤XŠ¿ã"¿"g¿æ(þ¦ä†¿ä_¯""e¿ã³Š§ß­¿áa{_ò®ß¿Ýé¯Ü|SAGNbcu2MASX J06533986+1636432?ïàÖ£	þ?fj>A›Ãm?o)\öê¦?fj>A›Ãf?ïøØ%ȟ0?qöÐbØ?LŸh݃BV?qöÐbÙ?ïÄf5÷@?|E7p'¹?}Ìþå_f?|E7p'¼?ïêۑ0h?T-¬uV?e$náϙ ?T-¬uX4FGL J0653.7+2815?ãCïXˆ˜@)ÚÑÐAÌSÀ:7zÀ~hÀ<U	Ĥà@G_ÏÉVv?üê"Ash?¾È"™"‰?Ðk/coæî@®þ#†î@#óï{x¿èÉà>¿j?°r@þç•ë¿Ò¾¶4žm¿Ø'=4p¿çä&Eüd¿ïþΈ°=AGNbll3FGL J0653.6+2817GB6 J0653+2816?Ûuc²ãsÜ?ËÑ¿Ö?âEN&ŽF?ËÑ¿Ö?èV*g–ÂN?ÒD콊"!?ΧVa¤öÉ?ÒD콊"!?à^ˆpaUá?·¥ìúõ>2?ßBï=T=?·¥ìúõ>2?ét	ú7?«j¨;YF?Ê/óØ—#?«j¨;YF4FGL J0654.0-4152?íÃ=Vü3<À1BjDAxpÀ;%ð†æ8¯À<"ľá@ ´£¶(@å¹}d¯­?ÄóSIS0¿¦	6õh?ãC
€òç@ƒ		i
?ïcÐT@Éõ¿åÖCŒ¿è"Î1&¿Ó–[@î\¿¿á¦R_Hdô¿×V%Pœ{AGNbcuLEDA 571171?ïýo8*×S?,¾[@Œ"?4†>©EWÆ?,¾[@Œu?ïýaÃ?S]ÆGé½?7ôñç3ãý?S]ÆGé«?ïöãyHŸL?_zÇË;ê¡?R9
nÁfì?_zÇË;ê}?ïòA?HA•Tc­"?[}Ä ü‰Ô?HA•Tc­±4FGL J0654.3+0923¿èét#ÙcQ@—ÊÂ0'˜À:¹C•%À<:̂úñ£@ 	Ip·M4@Úÿ•võ?Ä2T"Œó?'NÓLè?ÐA
œÛ¾@"²4°·?îQ.ƼèS?¡êˆtƒ4¨¿å
!AN¿â£¹þ"ï6¿ÚG5ß
&¿æ˜ˆAØg‹AGNbcu3FGL J0654.5+0926GB6 J0654+0925?ïön*e&/?Rãp'(?S#«5³¢z?Rãp'3?ïüéf×?Uç;%Àƶ?8·SÉ5l?Uç;%Àƽ?ïæÆOÒŠ?pè%z"0?i9°-ñtÿ?pè%z".?ïñÉõ•ðk?Kƒ5Öã?\lÔ'^?Kƒ5Öâó4FGL J0654.3+5042¿å×%͔œr@5ˆ‡"žÀ9qal+¢À<Ë­b@ê/o¯:k@™'¥R?¦æÏ=¦Ý?´%`Gú|@2Ÿà·ö@ð…×ÅÏ-¿Öü°?Mrпßv–_Ruï¿ãšÑ!Æ#e¿â³9žeË¿å«äT¨ÎÁ¿ïÿäQMÐmAGNfsrq3FGL J0654.4+5042GB6 J0654+5042?ïþBBÔë³?(mlM®hw?+ÛÒ±DÏ,?(mlM®gÞ?ïñ¨˜¾ë?|ÜM¸oˆ+?\®Îƒü+?|ÜM¸oˆ,?ï·ýªXJ˜?­Q¬vq?'•iíZ9?­Q¬vo?ïþy.ê? ©¶UA?(m_lX? ©¶T»4FGL J0654.4+4514?"z—ÿ'ÔQ@3cag#$ÈÀ8ë¤dζ²À;ԕ"´@?ƒ*+ù@vÞüz9'?§[ADT?´‹¿f\ÖE@{…L»@'M³çùy¿Üs k°R¿Úd_ó.á¿ä£PÂe?Ë¿ãHÑ?£.¿èåo®¿â	Y€ù»AGNFSRQ3FGL J0654.4+4514B3 0650+453?ïúÒdy?>×|ܤ"?D·Žn‡ô?>×|ܤ/?ï÷5(v͏?p!µ1´?Q•¯dà ?p!µ1´?Ñ}?…œ²hÉ¥?ˆû‹¹àí?…œ²hɨ?ïÿ×Û^A>êl²w~®>ôPßtV>êl²w~ª44FGL J0654.6-4952¿Ý}ãW`ƒ!À3è÷‡‹zÀ:™7ÿJÎZÀ<{OnÓr@JRÃFfA@:6\³_?Àª$@ÒA?š;aµ_?×e …±…@û7Ä<…?ïàÝÆTe¿Ž×GWµý¿é´V~'ÖW¿á	Ò¾@î¿ì˜n÷. &?ÊSØÚ¢"AGNbcuSUMSS J065518-495205?îö»³y'?œº¥GŠe? "DÈn}‡?œº¥GŠd?ïð†ý½Ó?{#!\e¢?_Øò"Zf?{#!\ež?îþʱ"?"ïr.Â? ^´ç¾[?"ïr.Á?ï¬Î¯N4B?qxù+ý'?"ÌT,rïá?qxù+ý'4FGL J0654.7+4246¿ä½‹6@2›ðgȗÀ:VÛó±=$À<XÌ'=«@ P2O2˜.?ÿ†'+½óì?¾K'Ð|°?±ôŸÏ"§?õÓ±Þ3ý^@Y?E:G?á5av<??ã+žI+Âü¿å(M[Óem¿Úà
Fe¿ä¡C§½¿ØÉB>=þ=AGNbllB3 0651+428?ïüjR_ÄN?6:ël—?<­mݗÄ?6:ël–ÿ?ïø‰þF?aLÅv.©-?MØÉÂâ®?aLÅv.©2?ïõ‹Íóz?Yß«¸J?TèdÁ	A?Yß«¸^?ï¦iŸÓü?qß«5å?†e˜<?qß«5å4FGL J0655.4-2631?³ãçBGçÀ%Ý)V:Ÿ8À:u	A}À<8$â7˜@JÎãþAº@KCË0ë?ÆHÆÃHi¦?ÉÙ¨¨UI@᤽º
R@(…a8ª¿ìS^¡Ëí)?ï÷Ìàméh¿â"¤¢Œ1|¿åF–Qæ|¡¿æìãË¿ÈÈf¶˜WûAGNbcuNVSS J065523-263041?îwέmX¨?¥²'^˨c?¨ƒ)*uh?¥²'^˨b?ï•tþ¶¤?¨z±±Ð.?Š¢ÀR\ú?¨z±±Ð-?탹x¥Ç‰?¥»~ð´\?³â4:Ñ÷?¥»~ð´Z?î§'0rl?'ŒtÁ}Ðd?¥MŒøÙQ?'ŒtÁ}Ðe4FGL J0656.3-0322¿î´¶ Ö7ÿÝ
ÍÞo·sÀ8S&ùz«À;‰ó3hã@ð¶ÛS@WwJº8v?­\ãã?ΔBWC@´'¾‹Áj@°'¹%{¿Å)̗Àñ¿á
Hï]¿çåàϹW¿é¤''¿ëÆ?wå¿ïÿù_|è3AGNfsrq3FGL J0656.2-0323TXS 0653-033?éäõ¢×ƒ?ÃØ…»µf?Èoœ)t¡ó?ÃØ…»µe?éì9÷¯É?Ñ͆}ƒ^y?ÈOè!@Ù?Ñ͆}ƒ^y?æ/Q"åS?¶âSô_ªp?Ó¡\Ø5õZ?¶âSô_ªo?ã¢Ñì)ž?¹ÚDÃ/í?غ\'ã¬Ã?¹ÚDÃ/í4FGL J0656.3+4235¿Ø_‹Õ…š@2Ó~=ÁÀ:³pޏmÀ<P%üu@ Ë­R3(¡?ÿyó$÷0?Æ>oçÄtå?º¬³æ?÷5'm,S@œèwx1•?ïù-Œ*E¿åùy¾‡å'¿Ñâ<xm¿áÄcq¿`¿æ"À%?nçcsdH AGNbll3FGL J0656.4+42324C +42.22?ïýyP ?5g»ødŒN?47~ÿR?5g»ødŒM?ïñû>·=·?}
Hú£@?\	''"É?}
Hú£@?ïõ|Ð+"ø?`5ZKt¸©?U_¨ö?`5ZKt¸ª?ïuÞGì<?xj1dOYe?'D7Šx?xj1dOYc4FGL J0656.3-2404¿ëËÈ4›1À#d¶0©À;("VÀ<dYV³jü@ €õQ%aŽ@ŸKÚÉå'?ÆrÜV¿H¿ƒ¢õ
ÐY?Àh[3,}@aþÍ¥æ¿æCé>GŽ_¿äڔk\om¿èI.p•¿£ÛÔQ¦eÛ¿ëlé7fž›?ÁÂkŠg¢|AGNbllPMN J0656-2403?ïó¾ßd»?Xñ)ÐN€"?Y܂A6ˆî?Xñ)ÐN€?ïúùk@?aiåîEa?DSÛð?aiåîEg?ïÂïÑßB8?€=öËÐnE?~ˆ^ãY?€=öËÐnJ?ïìQõKÛº?V¤šñ?c®
´$Dt?V¤šñ4FGL J0658.1-5840?ÊÂñQ²ŸÀ6 ÝDÀ:Ó"d®ÖÀ<šU¦$ÂW@Rmⱑ@S»¹/?Ã,hÿ?´ÂÖÿ«œQ?ðΩ+Ç?üäò7ëSÌ?捻å'6¦¿Ñݦ䱿ÛY—á]¨}¿ç¼o¢OJÁ¿æ¢nŠ!V'¿Äpêù³Š±AGNbcu3FGL J0658.3-5832PMN J0658-5840?ïìûÌP?\+V9ܚü?cû3¯àÙ?\+V9ܛ?ﳑõ¾2?"¾>&÷?ƒ¸s%?"¾>&÷?ï…!!O«Â?Šq{jKÖ
?Ž··¬Â?Šq{jKÖ?îšoÖíáÚ?‹*â¥\ðÿ?¦Y'!âc?‹*â¥\ðþ4FGL J0658.2+2709?ë_ߣ¹È@*ÍA·ZtÁÀ;½x›óÀ<…®
iæ@M†›@ì†;?ȌÇÀ'?yuD½®¨ž?ªLõbSmw@ÄØÆU9m?ïe€Âø¹¿×Ñ}
§¿æ̝Òä>¿ÔÊ#$G]¿é"Ì«>Þ¿Ü#"$ÓAGNbcuB2 0655+27A?ïèvåÄЧ?c¾áx"‹?g‰;/Xe?c¾áx"…?ïüŽÓ½yÅ?^ª×±,ý?;‰b1æö?^ª×±,ý'?ﶠ¬q?'ÿó0ëE¥?'WÔùã¼Ä?'ÿó0ëE¤?ïôÏÖUÝ?BßÙ´ ßk?VaüSTDÁ?BßÙ´ ßk4FGL J0658.6+0636?ëó'õ@â@j¶ÂŸLaÀ:R"ÅõB7À<+°¶ì'@ °jûw?ÿKXÃæt?Ã"ÝûsS_?¡¬ØwHP?ßmõܐ/@Ûäkyö'?ä'6ÎÉ&O¿ëów'1L¿Òˆ:̄¨¿Ú#ìnRÄ¿à¬![š[¿âžf½¤:ÝAGNbcu3FGL J0658.6+0636NVSS J065844+063711?ïó†cÏÀ%?S'/R?Xó8`¶g?S'/R?ïú¬Öw­?f}ª":§÷?EOô¦!IØ?f}ª":§ø?ïâëÖÒž?r6Á5B«´?m)-ù`È?r6Á5B««?ïõÌÿŸV?f‰[Þ?~%€0T"?f‰[Ü4FGL J0659.6-2742?ïÿ¿[^ÐXÀ%/UÞXæKÀ:3Æ&À^*À<3"'ʘ@X‹®õKq@ÚíÜçÍ?Â\ÉŃ"?Ӑ{xFb»@íÅÖ8†Y@‡¹Wzf?ïû7mª¿Ü´>¥¿ç(Ãm¨z¿èjÃQ#¿éÿcøÍܗ¿ðAGNfsrqTXS 0657-276?ïS§¢Õ¤d?™Ò:Í6<]?•‹¥Ks‡?™Ò:Í6<]?íÉ0ê(t?àzÏÑÚ?±¶x®¿\i?àzÏÑÚ?æ†O;äö?´ƒÐ,J5?Òóa‰ò6?´ƒÐ,J4?íâWævz8?•Nj p²?°í@ÌL.E?•Nj p³4FGL J0659.6-6742¿Õú65%À80…†"À;Z©Jç"ßÀ<¿<ÓÅåR@"0ü@ظ=?úƨZý|˜?Æuøˆ‡?œãg‡½gï?×p§\û®@á*ŽÉÝ¿ÌÁ¬­O"¿ïúeA"_%?ïú¹¤ÑÜ¿âït'ƒ¿Ü»©ú9íb¿›…
›tAGNbcu1RXS J065933.5-674356?ïþ"¨
ø?(fhMj¿?.¶µ ŒC?(fhMj5?ïý©Ë,ãV?a6¯Õ4èò?2±¦˜åLn?a6¯Õ4èî?ïòBÚÔ?dF1´ãä?[Ñ{ÞJWš?dF1´ãË?ïö'뢠S?F¯:Ai§|?RÜ(º¿WŒ?F¯:Ai§ƒ4FGL J0659.9+1709¿ëS;ÝüP@#¥ß"9çÀ:4\|ؙÀ<‰£–@(ÄBd©x@#«äøê?Áï,ž¯N?¢_ä°Þ?ÝÛB›Ûé@
=‰T'¨¿áë5@L ¿æDI,«¿æêò®~¿çbår¶¿ë	3ðÈT˜¿ïÿHë+\¥AGNfsrq3FGL J0700.0+1709TXS 0657+172?ïûedBè??Œ-'.k0?Bkænô`ƒ??Œ-'.kL?ïûø 1E?cõ¤h²Œ£?@Ã:çE?cõ¤h²Œ¤?ïÕ£Ly8g?t̹ë"?u.YÃcÌö?t̹ë""?ïûÿ§ƒxi?0Y˶ægn?@aò]þ?0Y˶æg4FGL J0700.1-6311¿îÀ½ÞR+·À7·ª%ÙÀ:±ñNŒU
À<˜M×ú'y@ )ƒ:1ª?ý'-ê
Ë?Ƃ_UÐìí?ã©'#V?ýÖ—Péý@ô
8"x¿ì(ǀ?ïúªùš‹¿Û["ÀĀοÚkaýËó¿äãacÈ&¿ìó)WèbAGNbcu3FGL J0700.3-6310SUMSS J065958-631238?ïüz»xdã?5Hnºˆ÷?<*$<ØÜ/?5Hnº‰$?ïûnaëy.?^·¨ûö?BFxRB&?^·¨ûö?ïܵ"˜À ?qBj/€Q?q¥5³Ÿ°v?qBj/€K?ïÊ 7àu˜?k[XÑè7'?zïäÅ3ü?k[XÑè7'4FGL J0700.2+1304?Ùhš%lZ@h>]2àþÀ9æGÁ_±À<(É Èb@Þcðë: ?þ«rßñm?ÀéðÊ1?¹ù]ú\'?û±ƒ›*"?ñºØ®'_?ëKg<O;§¿åj(3¦¿àà Ç`¿ÕZ¤k¿äÐeÁ•a¿Öi}±ÇAGNbll3FGL J0700.2+1304GB6 J0700+1304?ïâF™¼Ù}?gãrIºFi?m¹fC&ƒ4?gãrIºFf?æŽ	ž­#ý?ÒTÙ+4·–?ÒãìÂ¥¸?ÒTÙ+4·–?ïŠäËu¹?ˆÆîd›Ø´?FÍ"'¼¥?ˆÆîd›Ø¯?ã¨àô»l†?°÷Ω2?Ø®>‰&ò?°÷Ω14FGL J0700.5-6610?îzÆÁu=À7–6—lÀ7àóÌëÖ}À;n,Ñð"@zrè)õr?ÿlV…GÒý?˜´C÷ä?³èù~0²z@H	N][%@J	99²~?¢‹>šÖ—¿Ø}å,õ,¿àŠò×ùP¹¿áQ¦ é4¿åó`	€¿å™
Æ(ÄAGNbll3FGL J0700.6-6610PKS 0700-661?ïûAà8O?AŸ®ÙÞÔ·?Còø¿?AŸ®ÙÞÔ¤?ïíºå³<Q?t‹›X:C6?bELïy?t‹›X:C5?ï°bÐ!?‡'™Š"ì?ƒçK÷œ:?‡'™Š"ì	?ïàPÕÆõ?\?ôqkæ?o¯*9â
?\?ôqkæ‹4FGL J0701.5+2511¿ì¨JÏ2@*ˆšgó
À:ñ/¨;ôÀ<‹5RÈ$@!""«þÎ?ýïüÍE˜'?Â`#×·¿"€-Hâ$?ӋªãÃß=?ÿ8·§ ÀÀ?ç–_½Õ¹¿ë%d`ãð¿šÚ}xg¿éCN¾ÿږ?µÝ´¦M¿Û'@dtßAGNbcu1RXS J070132.1+250950?ïûlJ'm6?F?öü±T?BNÕöK(@?F?öü±2?ïûá@…º?d¨Þ"
?@zýéD?d¨Þ"?ïÒB‹;*T?vãVÉÈQ'?vÞºbjÖ4?vãVÉÈQ?ïê[Ø?Yo;xƒô?e¤'ôäò3?Yo;xƒù4FGL J0701.5-4634?æGs<¼À1´ÖÂïÔ9À8ýë7ñÞÕÀ;íhò1á$@àht³†@‰bI¡3Â?©¾X»æ?Äâçxb<@4aQJ@½©›ð6¿Ì~UE¿]¿áŒ†'ø¿å‡)õœÏ¯¿ç7?#Vq¿ìíÝ|艿ãšÑ½woMAGNfsrq3FGL J0701.4-4634PKS 0700-465?ïÚÓ(´2.?m¿$¾DŸ?r–k¥æé0?m¿$¾DŸ?ïóJ¥j´1?pã$ý£?Yjµ*— 9?pã$ý¥?îÙ´?˺?—ã	¶±›R?¢d¼D_B?—ã	¶±›Q?ïøAÈίT??tÕí%?NøÜÅB°+??tÕí%i4FGL J0702.7-1951?ë4¯Üñ¿bÀ_9K{)À8°µ "µÀ;q׉¿1@êwY¨½Ï@ ºK?©ôr-Dé?¶Í´~La-@
ۇz³%@b
Ë5¿ÐìK¢ë§Ù¿àÏ9#7<­¿ÞÕPߖ~¿àèuÕo2¾¿å,‡m¹—¿æ¢Òþ?5 AGNbll3FGL J0702.7-1952TXS 0700-197?ïþ2Á­r?%þ3¹–;ú?,Óå/çV?%þ3¹–;¥?ïû¥°¹·?X»llhª|?Ai?Ñ ?X»llhªƒ?ïÅÊëËêÐ?-/™É36?}Š
—Ö?-/™É33?ïüCL­"-?.ÐÃ6bI?=嚓ދ?.ÐÃ6b€4FGL J0703.2+6809¿î×®pt'…@:.Y¯ž¿À;Äp/=mÀ=y@]¾!@!m›
à?þÁX$"D?Í¿9?«BNâ™ÆC?ß:#<p@#_•'Í¿é(Qû,Ý¿ìÎÛÐuι¿¦èsFs­¿Ý»ˆÂ0ç~¿èóá
Ìq?Øߓ£áF,AGNbcuGB6 J0703+6808?ïÿ"ò¦ÁØ?70€î¶?¡«'ÅŸ?70€î§?ïþÍß²ÉÝ?B%]nm	Ï?#"Ób+
?B%]nm	Ä?ï鷐ôO?uŒxvb?fïHo±(?uŒxvb?ïû/ù§¯&?5fK?W?C@aCgñ?5fK?Ví4FGL J0703.2-3914?»L*&V)À-J×ùP¹VÀ9Àø£lŸÀ<6¦CÌ«@b'vŠv@|_ag?´ÂüÿÅr?°uŽbÿd?ûBJÈ{.u@Q&úë™?ïñöó4¿ãå"~°	H¿â´½ý&¿×ÇÚñR¾¿ç$¢¬gÒw¿ß	žs`AGNbll3FGL J0703.4-39141RXS J070312.7-391417?ïÝYN,?p4cBV†?qSXþiø3?p4cBV†?ïã8>Ìò?ŠEp°ì?lÇÁ3
â'?ŠEp°í?ïÃqdCò?Dv~ÌÊ?~zGMÞ?Dv~ÌÄ?îô…ÞIe˜?ƒÚ ­1S,? ·¢i¦Ž?ƒÚ ­1S.4FGL J0703.3-1042¿ç=¡>S¬–À'D`'!À9j‰r¡À;HlÞO¬@¶6]_,@5£]gº#?»€;"n?"‰y­ò?ÙSËäÅfý?õ˲BÝË"?ïìfZ§ìC¿»ª¾–9y¿ë0Ď9ê¿é;(àsó˜¿Þo+|/¦a¿Ô‡B^Ê:ÌAGNbcu3FGL J0704.1-1043NVSS J070322-104426?ï¤ÉÈê?›ò¬¿3'h?œ}ËfÆâÍ?›ò¬¿3'i?îÊ Bân‡?µèW´ªÐ=?£UûÑÙ£?µèW´ªÐ=?ìÈ(يâ²?£ºõ2ÈÐ~?¹¾¹3¨êl?£ºõ2ÈÐ?ê—FԄõ`?¯a¢¡–Ȑ?Å¢ä­ì*~?¯a¢¡–ȏ4FGL J0703.3-0050?Ä8'½7@ø/0oÀ9ˆ²1@ìÀ;—'?2D÷@dn9ïdý@ƒ¯à,ûâ?¹nÓâ¯|?É'ÄÀ
÷@~…vÌå÷@
Àöäxe¿ÝO©@U°Œ¿ÝÖ
RÎÙí¿áú4CÔk'¿ä>¥¢fqÏ¿è1áÏh^¿ï÷:Êi²AGNbcuTXS 0700-007?íüñ¡?±ø'Áöñ®?°wïŠ÷Q?±ø'Áöñ®?ïIPÿõÚ¹?±'Á£,?–ÕàD©?±'Á£,?êl=Nžm'?±tÛòX
2?ÆO
ņI·?±tÛòX
2?ï·Pùce?"¿'f®0G?Ÿéàӓj?"¿'f®0F4FGL J0704.7+4508¿å
+Ï[•@5I˜ˆøÀ:ÇG'u¦À<hÇñ›¹/@ŠÒ¬_Å@@Ÿ}i[?ƲŸzQC?¸fœ«fK?îÑ;ÇVkG?ú"#xÕÿ¦?ÑØ	âx¿ã¼Å¸ÜU¿åX•Wëy`¿ê	âÂW}ë¿Ö"%>(¿ïð4í0EAGNbcuB3 0701+451?ïÜ"ä—–?r˜ëO†[?qîñ´4¥?r˜ëO†\?ï ´åšÒæ?²Àç‹ay³?›écL¥£L?²Àç‹ay³?ïiÚušdš?Œå¥M'O?'ıL³lÇ?Œå¥M'O?îÅ?}n?Çüêo
?£¬Ž)0?Çüêo
4FGL J0704.8+4907¿Ïtˆ3<@6BÅ;ËÀ9äz[ñÀ<8>gCÛø@¦¼õ¿4^@'8å#Û§?µ}€´Elq?Ö=C­Sá@
bô ά¡@.-ú'ѿ͍òÇ]L6¿âu۞÷§l¿ärB¬^¿éÍÃ\Ⴟ彵½¼Ž'¿å°eùRAGNbcu87GB 070112.8+491056?ïå5­^Ý?p)øeÙ«	?jÊíR¡#¦?p)øeÙ«	?ïø69ÈÖ?j[70Ð8?O'ߨ©«?j[70ÐA?ï>Ë°PºŽ?yÉâ:?˜&‰õè®+?yÉâ8?ïñÍ¿'>?FKµA´ý?\d€Ýӄö?FKµA´ý
4FGL J0705.7-4848¿´õ1ÇøaÀ1Øc8´|tÀ9Ö­ò2qÀ;úˆFŠþÌ@âs'?	*@Oï0l¯?¶®|Փ›?Å?Û¢¨‹û@
3Xòà\Í@½^Ä»?â—m¿öûu¿ÔB±Á¯¿ãx†YJôñ¿åûŸíp±¿çŽëUN.¿ïþu]AGNbcu3FGL J0706.1-4849PMN J0705-4847?è'(ÏÈå?ëjNħÞ?Í÷\ÀßÄh?ëjNħÝ?ã	—ø£8?Ҏ˜[öÍZ?ÙÝìйŽ?Ҏ˜[öÍZ?êˆ	µ®š?±G¤däI?ÅßÃÙ)E•?±G¤däI?爨ý;¶Ï?¥†Ã0©ùS?Ð'd?¥†Ã0©ùS4FGL J0705.9+5309?î¡kâe@7€ZpŽÞUÀ:Ø	ٝ•¨À<³Ð¡m£r@ÁÂr«Ä@'6~AN?ÁÂ˗´'?¥ùiãÉh"?åe'
@ž3ƒ:1ª?çÛ-¸Ÿï¿×å°¿åï
¿[J)¿àñ¦&oÖ¿áúw?|—«¿å¡àåÞlAGNbcuGB6 J0706+5309?ïøv`‡:à?Fl?å7Ö?N&}ãü?Fl?å7Ì?ïþri4÷`?DÅæ:8>?(Ùl°‰è­?DÅæ:8.?ïï*Aa<ú?d"ǟäC¼?`Õ¾žÃí?d"ǟäC¸?ï鱖"³Û?Nø·)æ?fNiÝL$
?Nø·)æ4FGL J0706.1+0246?´%Q|'"Í@.beOæÀ:ýž5	ÍÀ<SôH;Øô@#½ÙI\ë=?ù"¡ò?ÄÚUv
Q?†o*bÝ£g?Â`|-Q?ùœÅˆŠÓƒ?ïMú^ÖO-¿ð?ïÿþó…õ?Ôr‡qxé ¿çää†&ö?ˁ%D@çAGNbcuNVSS J070610+024449?ïýÛôŠ¸?0lLA˜Ì?1 _+ªI?0lLA˜ß?ïï5Q·¤€?}xŒl p?`Ê®H[g?}xŒl o?ïÙ·iJs?x
ªãi'?s$|KZÆx?x
ªãi˜?ït­¡¹Üþ?‰ºXRŸHŒ?'jKÈÄ`0?‰ºXRŸHŽ4FGL J0706.5+3744¿í#`Ê9µw@2üð¸,,À9'dö#Þ,À;Ӝô—ìñ@ÍëZ×g?ü=³¥Ýu?«–3Þ~Ðë?°rõjû¡w@ƒZ'ó@=«2ž7ä?ïæ
öÔT¿Ùº"ÛÍпٔPdF{¿Ú&Y›|Ȩ¿Üž^$x…M¿ÞË(~»ÈAGNbll3FGL J0706.5+3744GB6 J0706+3744?ïѽËb<@?rI±Â­GA?w!Náà?rI±Â­G??íà UÝÐ?Á
°Ç¹`Ä?°þýQ?Á
°Ç¹`Ä?îx"›Båb?™ÿ±!_?Å?¨vÆKÑ©ó?™ÿ±!_?Ã?ì0afë¶B? ÉZgðÿ¢?¾|ôÈ¢Mé? ÉZgðÿ¡4FGL J0706.8+7742?»žŸ·ÅºÊ@;Gy¢ƒMÀ9kQÄòÀ<,=ÐE'Q@¯"}ûÙU?ýıû.·?­òŸïV?¾kdÒèoÁ@"ïï@Ÿ|󛘢¿ÀµÏš²sZ¿Õ‰æ]Â}é¿ÜÙhrLN¿ÜlÅP+¼¿äô,ø†Žû¿è"3ÿ
zAGNbll3FGL J0707.0+7741NVSS J070651+774137?ïý0WzF?4}ч=É?6}D/åÌ«?4}ч=¡?ïúQ…6Î?_ʽêzL?F»Ñë$Äf?_ʽêz[?ï…ØCz%Ý?Ž¦Á4Xô?Ž‰ï!vˆš?Ž¦Á4Xò?ïûù®ï2­?)"®$Ú,?@DC5O,?)"®$Ú4FGL J0706.9+6109¿Øâ¶6ñ@9^=áâßÀ:>pɖ·gÀ<'UÓø@¬¿y4t@,ÅZèƒâ?µ¢7¢Ù‰I?ËPÿT'?Ö<á>iÈ@"IX¹"?ï &Ö@¿äȒ@	‹¿ç>-—è¿r¿áÒ6™A¿ç}§á¿åmü\ÝQAGNbll3FGL J0707.2+6101TXS 0702+612?ïøíA?C}ABì@?LKâû…Å}?C}ABì7?ïýå¶Y?H€í³"U?0ÔOE>°?H€í³"U?ïî>n?dí¡
î	?aáÁìù'ø?dí¡
î?ïçßnÍ?TH«Ù Ñ?hþ '2ø>?TH«Ù Ë4FGL J0708.9+4839?ÛçUol"þ@6Ɉ;£D=À;IÐ&ô`À<Á½"¨™@!¾¢ªdm?ù~{?ÑΝœ…?Ãfmé~3?õslg@8Ë0šÂ¿ÛšÚŒ¿ïÏäM?êÏlº=~¿ÙèêÅ[>j¿ÒÝWžøS8¿ÞP?þªJAGNrdgNGC 2329?ïü_øŠŠÀ?6£±ó'p?=;«ª?6£±ó'f?ïýõž¹v?O¼C'^5?7 S
4Sý?O¼C'^ ?ïêQ¶6š?hvaÇ·?e®IÉeb?hvaÇ· ?ïê[ ,?W}aìrmò?e¤å_úÓë?W}aìrmë4FGL J0709.0+4304¿±Äž¤÷5@5-j½ãû½À;—ߨq£±À<žÌN!Ì@ N33²à@tÛ>—?̳Ä=19¿…˜ô`Ãô?·B›îœo@´h"ÿ‰¿Ø>\œŽ­¿î{ ŠN£¿°©»¿xS¿èä§՟Ú?¦RCí²1¿ïÿ¡ ÏAGNbcuGB6 J0708+4306?ïûÊ¥«lë?@Wٖå}?@ÕiRLO%?@Wٖås?ïþ›,x®?H<ÏBau?'&M8u?H<ÏBau?ïÎGQ~ج?~Òe¾¡?xÜW@"©¶?~Òe¾?ïýÔú^ËÒ?%–­Tßm?1X-	¡yË?%–­T߅4FGL J0709.1+2241?ëÒê]Cû@+ªºà;>šÀ9Hôá¾ÌYÀ<*2	@Êi©;ù?ÿí…tH§9?¯ΠÑ5+?±k
?-½S@t–'äZ@D!ÂóZ¿äÒ-^ÝÛé¿Üeށ*7¿Ýk¶Eê¿áK—þŽæ¸¿å_(뱔¿ÙQQAGNbll3FGL J0708.9+2239GB6 J0708+2241?ïþ'Z›¡Õ?‹t@¾Ä?&ÚVEâµp?‹t@¾?ïúãáÃV?]¡šÿ*L)?Dpxò§ù`?]¡šÿ*L?ïèá
×d?nŸŠâ#¨B?gáò(œ¤?nŸŠâ#¨D?ïý‡G?&âî{ã?3ÓÅÇ+E?&âî{†4FGL J0709.2-1527¿é˜§7Çå	À	0$öYŽÀ:–æ`ò‰À;øªLb@!€¼&'?ûÖNUÎh®?Á˜kܜùu?½j§=Ç
ì?þì¡c'v@Y1(¥¿ïÿÝ/ñ_S?ïÿþBe«+¿ÃGahz½¶¿ÇeöÔÞ¿åK
P»Ú¿¬:XŸ¯AGNbcuPKS 0706-15?ïþÍQ9¢?"-YÎ_–?#*ïeÑÀ?"-YÎ_Œ?ïðА¶ŠZ?"w;6{@?^^ޒëIÀ?"w;6{@?ïÃà…?ßüxƒp?~¸8=|ˆ?ßüxƒu?ïªäÃKÄ«?xFÂ!Sãd?…FÏ-Õz?xFÂ!Sãf4FGL J0709.3+0540¿ê'…"]³@@W_bf'À:7a=1¹¶À<1REG1î@KÓòZûÏ?ÿ»°åæyF?Ä@jS…ä?¸HQÓ\?õ:ðFN˜ê@'P(as
¿ïþ`ù?Ÿ?ïîLC¥q>¿çØ#­"2)¿Ð®#¿LÜ¿ãˆ$A'è|¿à8L­W¼AGNbcuNVSS J070916+053901?ïýÔzkd‹?/
"+ýH?1\,¤Ûœ'?/
"+ýW?ïóúž9Kq?wqäk7?X
Íi¿?wqäk7?ïÛ& ÕQi?z¡}]8X?rl¯•WJ®?z¡}]8Z?ïàñ%ñ†?^ñŸr¼"?oÚry"?^ñŸr¼4FGL J0709.7-0255¿ä¿Þí~@åc>"¹†À8†à66òÀ;q¡3ÁÎl@of×¥mã@¾::ŽqG?¥­ {\?±¹_°ƒ…@	•õB6Ü5@T84ÏÀr¿µVz\'}¿ß| $"I+¿åŽ¨orŒ¿âh‰¡~ëC¿çä¢ Ñ±¹¿ãHhÌAGNfsrq3FGL J0709.7-0256PMN J0709-0255?ïø¸Ì˜£?HàOçhû+?MϽmó?HàOçhû?ïÕÒ+z}?œ|"QýäÜ?uêqÂÀË?œ|"QýäÜ?ï­Î$+ø?…Å:5'Åû?"Œvõúd?…Å:5'Åû?ïýpwî­e?$§ ‹ÙÒP?4|@Š"Ö@?$§ ‹ÙÒ14FGL J0710.4+5908?îI±Û*$™@9lÀz®òÇÀ9ºÑ4:š0À<6ÙCӔg@!‰Á	u?ùâTÊ\°?°å%´¢"?¯9±$P@º?Ú
¢ñ@
'Å—j¿êŠˆ_	¥Æ¿´#7èy¦Š¿Ô$«°óRs¿Ðpeƒ<Šö¿Ü¡ººÑw¬¿Í_9÷GŸ§AGNbll3FGL J0710.3+59081H 0658+595?ïÿ!ÛF½?Žµ8?›Ä—(Ju?Žµ?ïüä¥P?RuÁ!ž@?;€Ú×¥z?RuÁ!žD?ï'?g·HEà
d?`ðèeoý?g·HEà
g?ïî)wZg?R›gÑJ?aáֈ¥™?R›gÑ=4FGL J0710.8-3851?ÕÐ:€¤ãÀ*E{cM­2À9œFp&ىÀ;æ~AN~é@õ£	ÚÊ@ž¥·µ?·ûRò[²?ÆRüýA@"ô%×*@²§|0R-¿á•ú=H_ë¿àƛÞÚ¿çöó<¿ê;3¢™Èi¿çʃÁd¿Êëï½<¶ëAGNfsrqAT20G J071043-385037?ïõ±lÒŽ?S~è^
Á?T&[ØãÆ?S~è^
¿?ïü–'Œ?S ™õ³?;OÇ;s¦â?S ™õ³?î/˜…ê"?˜+4àk?¦ýw¡V¶?˜+4àh?ïôHÀ‰8L?Gëv…"ü?Wn~íi…?Gëv…"4FGL J0710.9+4733?ï½ÿ$‹©P@6Ìt§qÉqÀ9ýçÆ²À<Owï$æi@¸Ä(äOË@ë꺝 ?»ËA1xö?Ãv.^b@*6âëC@y	³ˆB?ï!#}´¿æY*Fy¿è¿ÔáïÛ¿çq·20Ô´¿ð?ïÿÙi"A'AGNbll3FGL J0710.5+4732S4 0707+47?ïýڕE°"?7Ä{#¶ë?1+UÒ{^%?7Ä{#¶€?ïöɑ¹	$?€ø$ˆ?Rl܍í³ÿ?€ø$ˆ?ïXøVý¸?Žó]A»
?"àõ I(?Žó]A»?ïé.ӌ{?WÓ6#<GÞ?fÑú,sƒ¡?WÓ6#<Gá4FGL J0712.4+5724¿äR±í5ùð@9ZakTãÀ;s\,PÀãÀ<µîj¬FE@"(évј?ü-­$ß³?ÎRœ-Q?¯ÅHŸ5Û?ã?Ðà@ÿ'¸ÿ»b¿ç£æߝ‰é¿áÅâÝÛ<ý¿ïš@2 ?æÿOÁ^Y¨¿Õºt»=Ù)¿ÝÁ'œzIAGNbllRX J0712.3+5719?ïÿrYûeG?½sR,E?´À"W$ù?½sR-7?ïþoæ[	x?C–šÿw¦?)šOhkÑ?C–šÿw¦,?ïè?nxö«?tWN¥:ÓÇ?gÀ'‡	U?tWN¥:ÓÄ?ïþj@Ëb‰?#Õ>-#É?)[óI×j%?#Õ>-#ý4FGL J0712.5+3311¿ãéąç)@2Žª:э&À;€y1DFÀ<¤ªIë@ #÷êï]?ÚI…ÚõÚb?ôj\_|gZ?îûÀÖ…&?ó¿hæsg@˜'°H1ȿ畟¿MˆI¿é¸;Ÿé¿îÍD¡š™õ?éÚFsBî¿æPÊï¿ïú'`åóåAGNbcuNVSS J071224+330953?ïâ]ÕԎ?kÌàÍXÿ?mê¢*+pß?kÌàÍXÿ?ïü!™w¯w?Y4ãœ*[?>ó4B"74?Y4ãœ*d?ï9ÖÂe?ù 壺?˜Å<dz]Ú?ù 壹?ïýMêG®?A½`1ä?5«ã?A½`1ãö4FGL J0712.7+5033¿ïZú)û@7Ý÷¯îpÀ9ʉ%®À<9M÷×ü@Oô**¡@wڎVo?¤)#~¤?š<&]#?ón_ċµ«@®B"ùF¨?ïÿH˒:¿Þ±	!ç±U¿ä)S€°"ˆ¿ã¥Ž/L¿ã{A–£E¿Øºùe²€AGNbll3FGL J0712.6+5033GB6 J0712+5033?ïÿ)€ŸFì?Õ$6-?Ïì"~È?Õ$6-º?ïý'‰é[C?GÎp˜3z?3ë°µ%Ö?GÎp˜3~?ïéÈ·gpÞ?hÔ¥e$9?f7H˜!
?hÔ¥e$??ïþ1V-ñ?´™ô[?,ê ïÉ?´™ôö4FGL J0713.0+5738¿Üd…ˆüÞ@9wt¼j~úÀ:ª‹#À<[AE÷@sáo@Î@Ãa	/T?µ±¿?Æi†?µóãqT?þ! v˜Ò@úÿý{ÁA?íjAQÙçh¿â•?í«À¿åÒ<öˆˆ¿ã£š8ûÊ¿éf\፿ïȶ`x'AGNbcuGB6 J0713+5738?ïù,U?CevÅÓVæ?K‹ÃƒN¦?CevÅÓW?ïý¬yc?O~>ߤL'?7Jœ3ôç#?O~>ߤL˜?ïÕÙU	?sÜH/mª%?uwU{²?sÜH/mª?ïþ—·Os?1…{?&‹Ã?1…¦4FGL J0713.5+2537¿ïÉÃÛ\Ø@/Ù¾ôœõoÀ:¹×†d2¯À<ƒÅg}¾@¦¾p=«?ýǝÓ[\?Ðú±AV¥?Ò—ÀÑkî@Ÿ¿ž ß?üë&¢E?ïÿHµ{wp¿¹ò4æ;´¿å±æÍ)¿Õð9Õó<¿í¡Š~ɉ¡¿ïçôpÄÜAGNbcuNVSS J071336+254016?ïÃ-ô?‡Û]ï¯?~tiðøõ?‡Û]ï®?ëTo,ôw_?ǒ;ÇÙ?®CL."ƒ?ǒ;ÇØ?ìû©LOT¦?£ØÅúP'ï?¸"µ…Zá?£ØÅúP'ð?éyžCƒ±ô?«'¥DΗh?ʆññ81?«'¥DΗh4FGL J0713.8+1935¿î¹ü>¶¤‡@+'ãÑÌÀ8Ü#™b<5À;ØߑËnÿ@_""	"@-ÍbôÁÞ?ª";}üÒp?»	7¡¬ãx@™ûçl‹D@µˆMÁÔÌ?'%f ‡¨¿áˆÿ΁ٿå4ƒ•KV@¿åãÃb(¿ìçù¸¢ž¿ïúÈRꈟAGNfsrq3FGL J0713.9+1933MG2 J071354+1934?ïúckwl??‡=Õì¨?FrR"O¼??‡=Õì»?ï÷4*k&2?yLZ—Q+ï?Q—«)³žƒ?yLZ—Q+ï?ïgBIª¦ó?Žv=Ç!
w?"¶Ê«!}?Žv=Ç!
q?ïÿ²KY­>ùÕU'˜4•?|-)•b>ùÕU'˜4m4FGL J0714.4+1110¿Ò"@`z'¯@$H÷‡‹zÀ:Èû>ÐhÀ<rŸC@Ùî»4@¤XÍ?ÐÙ=^m"?ÃØáty¥?ö¡]b±¦@|Wt0('?ïýƒÿ("Ÿ¿ÝûÙ)Òa¿ádže0[¿×î,-…tI¿åŽœ`w	¿ïÿý¡UûŠAGNbcuNVSS J071416+110830?ïþ´¤-÷^?&'BÄ÷¡?$µ½ Š4?&'BÄ÷Á?ïöñê(Bò?gk߬éÿâ?R+¯z‹?gk߬éÿæ?ïËÌÿ%Q§?}%ŒÙÕÀ'?z€mW,Ž?}%ŒÙÕÀ+?ïÖ('Eéß?[
ٚpø"?tëì]æ?[
ٚpø-4FGL J0715.3-6828¿ïÿx›VÀ6øƒ‡ß\òÀ;i•ÅσÀ<xÉ7Ã@šh®ëƒ@môݍq?Ä<Dÿ¹^0¿œsY>	Ðä?Ø#"Øå@.`÷炱?蝷€µG?ÊOø{QZ¿é¥b$¸F-¿áÖ3ž$E¿âešŽŒ^¿Ð~Dß-!¡AGNbcuPMN J0715-6829?ïêb(vC?f†"MÎ	¡?e×ý‰¾?f†"MÎ	 ?ïýpO¼}?VÈB[ß|N?4}'
R?VÈB[ß|I?ï­úY~'%?…F˜úI?"i v6;?…F˜úE?ïíØ®F]v?QÂdŽ-È?b'Q¹¢‰¯?QÂdŽ-Ï4FGL J0715.6-4528?äþivÀ.
_V§¬'À:.ÄBº³À<S"}¨¢K@ïE…pB@=Uæ¼b?¶šõº¿rdœBÞz^?¸"~!™ï@wNö³%1?ïõÄr‹7׿äãü":µ¿ä‡.]
¿åÓPÊï¿ëüœ#·•?Ûáad°AGNbll3FGL J0716.0-4525SUMSS J071544-453031?ïâmD¥×ß?m"OW\Å?m'»Z( —?m"OW\È?ïüÿ¯âÌ?S€^$3ŽZ?8€éŸÐ"?S€^$3ŽM?ï|Ãø À/?ŽP)¥Ý߇?g€ëçùê?ŽP)¥Ý߃?ïêym†îé?U1É
/Jn?e†'y7?U1É
/Jh4FGL J0717.7-5519¿èÁl¶%D€À2zîÇÉWÍÀ:õÈ	ïmÀ<ŸµV¬µ@ úÿ£8Ô³?÷´º6È*?ÒÉu)wȎ?ÞÁS<=@âݽµØ•@·a·?Ôúß?ï]'îY¿äÎ˪Þ?µn˜K»À¿álN']‹¿êÜUÁR›-AGNbcu1RXS J071745.4-552024?ïŸ.¿þ^?ˆMZ˜I?ˆ4xPh;?ˆMZ˜I?îÞJ¡_6?¶èˆÜèZ?¢Uêì›?¶èˆÜèZ?qÅÁ?š€•â¸?¦öîC¤?š€•â¸?웣[;j?¥_Öno1?»"å#†$®?¥_Öno14FGL J0718.0+4536¿éêOy)¢@7tàP7PÀ9ÃJZ—%KÀ<G'ñ·gá@Ls 3&@û¥»ç?²°Õ_îR.?Ì-˜ªwŽ@o1'Y4@*€='(?ãRâ/àm¿Ò]³ß@¿ç4~!nÑ¿ç ÐàWÄ¿í ìt2¿ïúöv'"AGNfsrqS4 0714+45?íøÔï	T?ª¾)é»7Ç?°9X‡³õZ?ª¾)é»7Ç?ïìtÕìaã?‡ë¥'©Ûñ?c‹*žx?‡ë¥'©Ûð?éû経Ò?«1ÔÔº?Èc±)̸?«1ÔÔº?ïÛ!¢yè?[ç´	+?ro.øÃ
?[ç´	$4FGL J0718.6-4319¿ìÓÁZ·#NÀ+OíA·ZuÀ8œT§!A™À;'³ k°@ß¥ídó?ü¨J¡äÁ¶?¤Ÿ¨@?O?¸‡žß–ä@€€B_@´ jÓ?Õá¼'-@¿Õòâu«}È¿Ý÷:Ÿ
Kî¿ÕÚJ¤>
W¿âŽÌ¡ƒÈÍ¿çÈ}GS{¨AGNbll3FGL J0718.7-4319PMN J0718-4319?ï/nS·
?œ^SŠô9å?š5‰]_?œ^SŠô9ä?èØ…òtX?Ѭ½ÎöÚq?̟µè6.¡?Ѭ½ÎöÚq?î	»³}5M?£{ÖS  )?¯dDÈ,«/?£{ÖS  *?æ\ÎJ»Õ?¬#H¦O¯=?ÓFcj‰ÄT?¬#H¦O¯=4FGL J0719.1-7055?ìèËÀ7R™ú©vÀ;Ø©yámÀ<£Vh•ì@ '—)§Ä?ýá¥Ãsˆ?Ìý™ô2ld?ÊáYv¾Î1?ý§Ww¶@`õÏûUv¿Æ¯h¸P?ïÛ }-¨? 2=ûõ?™¿Úoø æ¿ç;Mlš]¿Îyz?a>ßAGNbcu1RXS J071910.3-705411?ïàmlMê—?hݸ­>íì?o'"²hr?hݸ­>íé?ïæu7¢æ?'%ÜÊqÀ?iŠÈæ]¢?'%ÜÊq¾?ï'e©Žo ?"#_QYJ<?‹¦•œdä?"#_QYJ9?îˆÍÒ÷2?•+#®µt?§s&"ЌÜ?•+#®µt4FGL J0719.3+3307¿îzl¡HO@3Ü£}™‰À8‡Á*[À;§Ü®ÂË@1<¢ô@¨l›3͍?œRiH1á¾?ºctïk2S@ 4çhY†@cÇ8ä")?psecÜô¿Ýû÷|ù¥É¿â­½½æ*¿ä0Ž]{[@¿çTèÅP׉¿ë`B5ÃAGNfsrq3FGL J0719.3+3307B2 0716+33?ïênbQR?bY¬x»r?e瑝®­?bY¬x»s?ï›ÜI؈?¦›ÑïDy?‰ú-‰Þ[?¦›ÑïDz?ï¬ãv"3©?‡˜ËJžS?"Ç"Zó|?‡˜ËJžS?ïôh×Ö¤?L>0¥r?W.üPR·?L>0¥b4FGL J0719.7-4012?æ×$ÃhÀ(VȒ«hÏÀ9¾Ò–³5À<ºö
³¸@–R½<6@x+h{?¶é±4v?®ò«â$*Š?öê¹aµý}?÷HýLœeÒ?ëG†Â&€¿ãr
™E¶Ã¿äÑ[ý¬¾¿ß ϧƿäퟫ+'U¿êi>]ˆÇAGNbll3FGL J0720.0-40101RXS J071939.2-401153?ïÕUl!?jσÖælŠ?uUtÉño$?jσÖæl†?í's"\»?½xé1»bü?³lc]'v?½xé1»bû?öؙ?ˆ°,¶?¦?Ö½Iه?ˆ°,¶?§?蝕Jîô?­YµÎû8?͋ªÔD1?­YµÎû74FGL J0720.0-3507¿çþ㢖þÀ#ÈîñºÂßÀ: žóu®À;ýPMö-@ѯJ/ùî@økú$ì?½	§ž•?ˆ1È=à¥?ËnÞÅr»^@©èsFs­¿À"dÌ2s¿äK G2Äx¿éïa|¼¿äž{`sˆ8¿à'ª&¯—2¿Úk	Cº[AGNbcuAT20G J071959-350448?ïü™DY<?8d	kZ>?;5Ý7'Ë?8d	kZ>z?ïÿQNôUñ?3˜.—¨
?Ö!uAì'?3˜.—¨f?ïÌࢻ?yY!˜»ƒ@?y®ò"~?yY!˜»ƒG?ïÿ«Ãñµœ>øÇÐ&ˆ¤j?'™y>øÇÐ&ˆ£°4FGL J0720.0-6237¿íZâP¡•À4¹"åûqüÀ:1SÃÌsÀ<40i@µ—;ÆU@¼›"Ud¶?ÇWèߧðÊ?Ï5E‡Á?ý5Y~ —@›èñƁY?îó‰p"¨¿èyÂÅâοí5#ÞV¿ìÌJ@•òE¿ïÿv}_Ò#¿åÅ2à'AGNbcuPMN J0719-6218?ïúÌ1ÚÚd?Ni'b€h?DÏ8"–sV?Ni'b€u?ï¯ñõ&'?™5õHL?"'»ö[A?™5õHJ?îRS"aÿc?›¿Y…ª;?ªÚÆÉà	Å?›¿Y…ª;?ï[®I70Ì?"ÿ¿ø\?"Š6Ùæy?"ÿ¿ø\4FGL J0721.3-0222?¿êr3¿@2Üû:À:ØúåäËÇÀ<b7£Û;û@!
ÂFá'?þ-î \+z?Æÿt>ì$?mWtárÏ?"VdnÆ@[Ž(¢5Ÿ?æþåþ÷í7¿îÏ
)N­ã?ØâõãÇe/¿åQ¯õüpÿ¿Ø©`Ó)ˆ¿À°{±|9AGNbll3FGL J0721.5-02211RXS J072114.5-022047?ïûwtãøÝ?Mvò'Ù?B",p‰›?Mvò'Ùy?ïþÝ7ŒE?GÎEª4èL?",‡;®ßð?GÎEª4èi?ïßÄÚ?ä?zߤPX?pw'à
Õ?zߤPO?ïõpÕÐxÿ?FÇ
d¹¤?UT_]?FÇ
d¹®4FGL J0721.3+0405?â×3€Y
)@!.3ïñ•À8îH[¹d:À;Ö@&t@™`ùj½@}ÝÙdŠÄ?­Ù=ôWUQ?ÀtƮЍ@u–AöD•@à‹†"¿Å.ld'5¥¿äÊf¿ç5ם‹@»¿çÿ©-‹S†¿í¡#›æzô¿ïÿç<t%AGNfsrq3FGL J0721.4+0404PMN J0721+0406?ï÷(Ù&éø?T‡P…1?Q®M²,ª?T‡P…3?ïäÙ?ƒAk!ô?k€pû&üN?ƒAk!ó?ïˆ!Íw‰?Šrònòd£?÷Œ¢»÷?Šrònòd¦?ï»KdØîš?j¥k‡%Wí?-&ÉÄYf?j¥k‡%Wô4FGL J0721.9+7120?롆¬ïï@<»à~íÀ6CÀ:Ð{?;2@e°Ñn?ÿÇ@ÿ¤?'AçÅ?­ÄÑ<w•@"¿U›=È@§6ÀÁ&¿¹.CŠCeZ¿Û3ÀîÈ¿âJ'Û¿à£W±—½¿å›aðµà¿ä1Ÿµ<OAGNBLL3FGL J0721.9+7120S5 0716+71?ïä^'ŽÉ?nënxƒ?k¡ïØq7×?nënx}?ïÚgï=Y•?‡ê™4ÓË?rÌaS5F?‡ê™4ÓÍ?ï)JXß?¡Zêl]?ˆµ»íiÇÉ?¡ZêlY?ïòŒuôN?Q^•Êu?[ðçd ?Q^•Êm4FGL J0722.7+3606?ïð×>@1@5ZÀ?öÀ:¤p¼*¾À<xåÈFUO@æ‡ÒǸ'@ـõ]åŽ?Åã!wôÙ0?¸ÔÈnÄ-í?ðdåÈFUO@º8	0Ö?ï—ùá­Ún¿Þ—¥ãÿÄF¿é¿8ÇǪ¿á)Œ 4Rî¿ïý
í™Ëï¿àIí>²B]AGNbcuMG2 J072255+3606?ïéöºªH™?mÕ.¯Dk?f	EU·gŽ?mÕ.¯Dp?ïãñü'ú?†™'"[?láØ ?†™'"[!?ï˜í)"ÜÂ?†•·ÂYÑ?‰Äµ›Ï!?†•·ÂYÑ?ï—D÷Óâ?uDXÜke¥?Š.Â<Ë€?uDXÜke£4FGL J0723.0-0732¿ïSò"#O@_9K{)À9äٞlg1À<±KgŸ@,­†¶h@°››ÒXþ?ºu…NQ?¡£0P¾^?èÍm¦Ìˆ@º	Å{ ?ï‰>½ªðÚ¿á{0f…p¿åÅ$aß¿áKñpD¿àÈ.3ïò¿Ù¬¾Å"3‡AGNbll3FGL J0723.2-07281RXS J072259.5-073131?ïÄùŸ¯1k?s¥F°Ãzý?}ƒ0(gJ"?s¥F°Ãzú?ïïyçøï|?'
OpÀZ›?`†…J?'
OpÀZ›?ïŒËz¯³Ö?Š©!uáÅ?ŒÍ!T
å?Š©!uáÄ?ï'ÏJÔ?síõõiZä?‹Œ-Jû8ƒ?síõõiZå4FGL J0723.4+5841?ÛÙi=~Ü@:ÿyB=À;å¼i¨:FÀ=¾@Bo@"{é~^TÊ?í@*ýڋÒ?àfQÒ[?æÝñLÞÕä@È¡#і`@a«ã=?ïÿõÿ 1#¿ç²›"nÝ-¿ïÿÝÀåãÊ?ïý¸Ý¬˜û¿ÁSIÔ	'¿Ø=ª]yAGNbllRX J0723.2+5841?ïõ¡%ïÛS?W—¦ÚÃ?T½´ IWA?W—¦ÚÊ?ïúgmßaÁ?d*V)?FbH'xü0?d*V)?ïv…æ뤅?ŠÛ%A¶_?'/C"‹oD?ŠÛ%A¶`?ïðÒH¶ô!?^cv3BCP?^[n'¼?^cv3BCV4FGL J0723.5+2900?â
w…Ê@3AƒÆÉ}À:¡4êÃWÙÀ<h"»@}¾ýVW{@iüp?Ð#þA¹Þ³?ÁfbÍT²?ñk:á}^@
¤ý·PcÆ?îáßeUÅ¿ãô®ÞOV*¿ãôC¾ñ—Ý¿ê~è=k›Z¿ïõÉ{´Ú¿ïþI¡ßŽEAGNfsrq3FGL J0724.1+2857GB6 J0723+2859?ïÿTßqî&? …4³}æ•?dÂ;P ? …4³}æ­?ïû 2G?_éº
6â¡?A}û6áŒ2?_éº
6â'?ï¿sÌ]gc?€–°c"à?€#è¦'š?€–°c"á?ïô|Ü°ÿ³?Bz…ô`¡™?WFžšv?Bz…ô`¡'4FGL J0723.7+2050¿ì@½È•V"@07!-w1À:Zڀêv+À<c" ³Ô®@ £ˆ6šÆÀ?ÿkªs±?¹*Â÷6ð¿¡xô2—Vô?ç:ê _@ü°­\o¿ä›?î¿åôi"PY¿âA¥¼½‹¿ÙɱÅ	‰ì¿ãêÿ½ºá?sKç¢ËAGNbll3FGL J0723.7+2050GB6 J0723+2051?ïù±ŠH ?@~µr²(¸?I9×Òß}Ï?@~µr²(Ä?ïùzêžo$?i€ÇÐ
O?JU†Cq¿?i€ÇÐ
P?ïòT=æ4?hœ"­²!/?[ÛW"3–d?hœ"­²!?ïá3òb,¢?Z{^‰žËØ?nÌ
Ó]Ð?Z{^‰žËÎ4FGL J0725.2+1425¿ë"à-qš@+Ó"Àh¡À7ÝàÇU•À;‰¢TS>k@4#.XX@ —Œ™?—ÄCøc®?°²œøž¸@AbÙ,@¬¸ú²ä¿Å"V¼OQ¿áfÕÂ>ÔQ¿äËj—MŽÿ¿ä
оsæe(]í!¿íƒá¡p'°AGNFSRQ3FGL J0725.2+14254C +14.23?ïýiaRÄ?0t­'ìH?4´õoyÜ×?0t­'ìY?ïéðÄ-˜?ˆ!c˜.·?f~;Òi?ˆ!c˜.¶?ïÝÜâ¨ù?stZÏ£¾)?qŽý+ƒá?stZÏ£¾,?ïÿÛö|\>ê(>pwë>òÁÿQ"á>ê(>p{U4FGL J0725.5+0216?ØÄÅäœ2Ô@!AlÅûø4À9Ò¹
x)À<ñü1>f@
Â
|?ÿ1³¡'œ'?ºÇð-"£?³¡ö4z0?úqºÝ¶ÿÜ@ÑîøEÌh¿àã£=‡J¿Æ(G‡S¿ßøÔ<­°R¿áAn?"՘¿Ü/0Åпæ%Pò`ÛAGNbcuNVSS J072534+021645?ïúöÓ©Ú?B 33pƒ?D'¸±Xš?B 33p…?ïù©Ä¢â"?ab‹,|²€?IXítws-?ab‹,|²'?ïá·Pnn"?sÃ:JGY?nH¯''n|?sÃ:JGXý?ïäzs<ÄQ?VWâJ¶G?k…ŒÃ;®ú?VWâJ¶P4FGL J0725.5-0504?½ ŠG_ñ@í:>À/0À:Û_D35·À<BxÔ'4!@!THÈpǓ?ÿ¯®(œ×<?Ãs…]Íf¿Ÿ¯¹|Ê?ßÿ^¢Í @aW<|Þ?ïõub'¬¿ár"›R×=¿ë*:э%î¿Ò¹'"µí¿åµ(€Ò£P?™òåæ#`AGNbcuNVSS J072529-050338?ïù»–ÏɁ?E†Ö"¹r?I¤ÀÙûµ?E†Ö"¹u?ïè9Zdë¹?'Ø/òŽ?gÆ¥›G4?'Ø/òŽ?ïã¤!÷oë?nì¡	G?l[ސh?nì¡	T?ï ö"Æ(ô?s÷'Ú<Ô?‡ÂZÎuÃ%?s÷'Ú<Ô4FGL J0725.6-3530¿ïª>°f¼"À"gn¤"ŠÀ:Åõ´L£GÀ<!6ãÁÛØ@ 0Î"oO@Ãlß&k¥?Äí&ο ÏÉ£Äã?à'qßÁ@Fx	|?ê'ݝ'A¿èæT]Of¿êýÑb]ÿ΁¼ÙÏ|¿à'8¾né¿à:Ã_æš~AGNbcu3FGL J0725.8-3532NVSS J072547-353039?ïýùGF?,«œºœéÎ?05ÅÏs†²?,«œºœé‰?ïþíäŠò¶?@M§€;B?!!·PÔ§"?@M§€;9?ïèSM«'?o°Ãg
_?g¬á²Tmß?o°Ãg
j?ïúËg՚_?6p»ž?DÒ`©–|'?6p»žþ4FGL J0725.8-0054¿ã&w9qn
@ñµ ÝDÀ9@†ºŸ¤À;ûbqåª@k¶ÓfD@£ì¤©(?©¡ÛÝ`î­¿"Fù¨fÕ¼?ê':…7@–¢n5é¿áaÂÈg¿áµ2Ùà¿âíp3Sê¿ÜŠÛ»¨N¿á%_Ö)lá¿Ý×_¢ÒÓLAGNbcu3FGL J0725.8-0054PKS 0723-008?ïø÷eŽ0(?G"³-)¤?L"iÇ?\ù?G"³-)˜?ïûÕ­=-?a÷;ûf'?@«‰KH4?a÷;ûf.?ïð×Ýzeà?hˆÜ#[?^PE4@?hˆÜ#[?ïïΝƒ>¬?OKO¢sžç?`1b|ÁT"?OKO¢sžÙ4FGL J0726.1+8114?æ––"'@<ÊÙ­…àÀ;çè:ç\›À=#Èb±@!r˜k?ûkëšî-?Ô)|»'gÌ?Äseè½O?ð<÷ØQì@‹cöÊw¿ïÿÿ)@k*?ïÿˆ¬Œ%?¬,©ßÀx¿Ú"s,G†§¿éôœßõ¤?ވ^Þ²¨^AGNbcuWN B0716.0+8119?ïô!Ò=´U?V—0FS\i?W¼["—Sÿ?V—0FS\g?ïóªZp?ƒÕÃ
x‡C?YÜ«ÏK 9?ƒÕÃ
x‡C?ï5:'j+?èbMó?™\x­Òº¶?èbMõ?!–ê?z앻F>ú?‰˜7¹ZEÁ?z앻F>û4FGL J0726.4-4727¿Çú"¬Z܋À,J ÊæBÀÀ9$ü!N.aÀ;ÂÁÀ)P[@T!¾@Âé@?Ä;-Ó?°s‡Ù~?¿úš ¹D@@a~ @Xj1Ϳ΋ÜÁ¸r¿ä•¤ýzꂿåÍùƸ¿çŏc}(¿ë—à±Ü¿ïÿÿ" 5•AGNfsrq3FGL J0726.6-4727PMN J0726-4728?ïûŽ™£ÓÑ??…Odx…?Ařp°À£??…Odxi?ïûÒÈ¥?T¾ù2M-–?CÌ´Ýl¨?T¾ù2M-¡?zš	?ƒØˆ­?‡_~aY~?ƒØˆ«?ïï`®Â9?Lô],O?`ŸQ=Æûþ?Lô],Q4FGL J0727.1+3734?ڟåtª‹ö@6Êÿ:Þ"`À;Á­!5Ú­À<é°¤xí@!À?ÒþÀ?×fxÚÝ0È?èùäÝå£Þ?ïûÙ_'F—@~†T@wUCÿ3Q¿ë?.Ö­ ¿ë¹‹§i¿Ð'4è¿ÙcÍÚ¾Òä?¾°»Ê²¿ïÿýFKêAGNbllSDSS J072659.51+373423.0?ïærb诼?lWaï%?iPD^?lWaï%?ïüm‹$??U©%m¯Í?<"¦ß†H?U©%m¯Ô?ïd{ö§yR?Ã"$Є?"p+Õ¢?Ã"$Ѕ?ïõv+ö?Uü©òKgu?U©Ņ?Uü©òKg4FGL J0727.4+5325?çŽ2)É@:²v‰ÊÀ:íâXOLÀ<˜V>Ðö'@'èZÔ@ïd†'V?ÊJàc'†X?ÄO3Cú*Ô?õˀœ?üåàaª¿â Aåþw¿æ½£Ï}5¿çFÓ#(¿æ~'bEo¿ìmå€ø¸ä¿ïÙuQ»´wAGNbcuGB6 J0728+5325?ïy>½¾ªó?X5í#Ô~?Ø(H*¡Ã?X5í#Ô?ï
\FZ'?­TëSêÒ¨?ž^4w4»?­TëSêÒ§?îôÏj½ö1?•ÌÚD¤³? ³	T œà?•ÌÚD¤µ?íàœ7¯
ƒ?šÛ0&9 ì?°ûB‡"ë?šÛ0&9 ì4FGL J0728.0+6735¿êsHëã@•@<e#'Õ€À:D6•¾BÆÀ<vî>6œt@38¬nÞZ@ñÈ`2p?¾š%@èc½?«Ÿ!ÃÊ¿?æ†DhÜ
@`«fuªÒ?ïV*
ðƒ‹¿è…H©¼ýL¿ë&àtI}ø¿íecœ‡Š£¿ïÿž{€©ß¿ïÿÿÊPËAGNbcuNVSS J072854+673225?ïü'Ð0ç?CÅ.ó??ƒi~xÁê?CÅ.ó?ïŸnSßÚë? o¾A¹ÜQ?ˆ$k	E? o¾A¹ÜQ?ï­¨×x,®?'Ž8?:³?"•Ê!ôÔ]?'Ž8?:µ?îçÈAîS;?'wz.Œ°Ó?¡ƒ{áÌw?'wz.Œ°Ñ4FGL J0728.2+4827?ïòQs"Ûâ@9Òe8hýÀ:´w
}—À< ÝÆT@Ÿ1ƒZ¾@'Ê<ϔ'?Ã;äI·¯?±êÄÚe?î5r£‹‹@yþô'9¿âwÉЙ
(¿æÂ
÷9‡á¿ÜZ›âŸ¿ä &æô–?¿ãø?"û'¿ïô ÞÇÌAGNbll3FGL J0728.0+4828GB6 J0727+4827?ïób'epë?Uû¦Ôî?Y:û5*°?Uû¦Ôíÿ?ïýyòél•?JçÌ;-?40h´›K?JçÌ;?ïÆ®Ð'g§?€}(j˜i?|¨—ìL+'?€}(j˜i?ïÆì·Ÿr?e4ãÓԑ;?|‰¤y°G~?e4ãÓԑ:4FGL J0728.5+6128¿Ô@î@;ûd¾ÆyÌÀ:b]¶ŠkÀ<üýíI@%DĀ"$@\»‡*+?Ãe4b2O3?Ä´ú<ü¶?ýR;×F£R?ÿ®B0èU¿àtéa#q¿áÌ{n5gÁ¿éޠ4¿é'Öt{'¿ïï{ÎRß¿è!^™HAGNbcuGB6 J0729+6129?îeäÆ\k?ª'*±u¾?©¡¿sš9\?ª'*±u¾Œ?ìüšbíÏ?Á±A6çò•?¸/|葆?Á±A6çò"?í´Å9CP?£†r37ØY?²YÖ5å4?£†r37ØZ?ëU,w«åÔ?«qґïÐv?«N!Ph²?«qґïÐv4FGL J0729.1-3131?ïðÑžjÀ<¹½üOqÀ:CTY©À<Wۉ(2@RG[^JŽ@À'¢Ü?ɸàœ7ƒ¥?¾JÍْ-?ðEUDÖ@JSÆP±É¿æ-z¿âp Ñò&¿æQøàüڇ¿ÝÝç;ãÛÝ¿ïþ¸Ø#B$?ïזàÜAGNbcu3FGL J0729.5-3127NVSS J072922-313128?ïðvêS[`?d$ŠjÈó`?_+YI?Y?d$ŠjÈóX?ïê¹nW*Ž?"bk}Š¸#?eF'¨Õq‰?"bk}Š¸%?îƱRü?™ ÃÎ(Ðl?£Ç"êß@D?™ ÃÎ(Ði?ïÅ›i3ù?qÒ®æá\	?}|2Kf?qÒ®æá\	4FGL J0729.1+5703¿ïì|™—0`@;'ýq?À:¶nÒE²'À<—…\˲ñ@V±<£@ƒ¥An?ĝ•½ ~?¸Ø›ž<Òª?ñvÙ*© ö@ïéW•?ï¼ÊUú˜¿ÑÛiþKtó¿ê=7˜ól¿ßJ(B>hñ¿í­ÞA¿=¿ïø#'¬?AGNfsrqTXS 0724+571?ïö\ü3½ê?U·ˆÿª)®?SF˜"+x?U·ˆÿª)¬?ïþ&+TÞ=?IéAîö?-J²ö?IéAîó?ï¡äWwKe?"ÛŠA2*c?‡†ê"-&ˆ?"ÛŠA2*f?ïòaÏd'u?JÔ¦ ñ`?[<a6û÷?JÔ¦ ñu4FGL J0730.1+6852¿å*ÆZIS@<¢5¤À;ôrKvö×À=x,æ0@`ú'ùÄ'@6âÔv?Ö&DÉ^?íâþ1ɦ¨@u-fj˜$@~=F\…½¿ï÷Ìàméh?ì¦-['Ý•?ÏÝê@ûó¬¿äîÝ}I,¿ïe©!ÌÙb¿ðAGNbcuNVSS J072949+685305?â H`>?Òßp*ý³?Ú¿o?ñՅ?Òßp*ý³?âcõ.G&?ÕMÁ£fJ?Û8£qõ²?ÕMÁ£fI?áÄ¡ñSˆ†?¾7Å"ÀÍ3?Üv¼Xîó?¾7Å"ÀÍ4?Ë#¦þ àä?°·{--Ûo?é7@WÇÇ?°·{--Ûo4FGL J0730.3-1141¿jfM®?ý@	ì:P]æÀ6ÂôÐ÷Ô¸À:ïø»h {@ÓÑ3¹ÀÖ@ ŽÉ[ÿ?ŒS¹Vç?·5Ed8@'€2¹¯æ@ç÷¤'Å:¿¾>Ž;Ô¿àñKÞ'ñ¿äÞDÄU/¿ä"BO/èü¿è=N	xNÆ¿ë÷ãœ*ÙAGNfsrq3FGL J0730.2-1141PKS 0727-11?ïÐx—ç?tÀc*?wÃþs4r?tÀc*?íÊvlëÀ­?ćoVߔ?±¬L˜¡ú–?ćoVߔ?龜‹«°?†ÕäˆÐx?†ÝÝ=»?†ÕäˆÐv?ïòûË˨?˜{,Ìä?Ÿ ††Šô?˜{,Ìä4FGL J0730.4+3308¿ëë0CÆäÂ@6NÆ6°–À:D¿Z'ÈÀ<mÆ	d-@æu27}?ýˆßØBKÕ?ÀA«›úœê?½T›bÇuu?ýƒ«kS51?ü8ÀA¤¿ï{œŽ@ ?ïñ¾>¶ì¿Ý!_€îýÏ¿Ô É°·¿ä´êÓ¿åÀ_–¾sAGNbll3FGL J0730.5+33071RXS J073026.0+330727?ïïV^—¾?`ºËOªì?`©¡ho@Ä?`ºËOªè?ï
Úeج?³úy"Ћ?žD³Dê~&?³úy"Ћ?ïÉ`\E±å?{ªœ¬Å?{OÑÝ'›?{ªœ¬Å$?ëâŠT)›9?¦é*ǀh?ÀuÖ¯Y"?¦é*ǀh4FGL J0730.5-0535¿é"¡œ´=@Xr)é–À9C_V§¬'À;û[Ð
nï@Oªú•@(šE'É?±ŸÑÛÄ?°ë	_
´@~%ŸÌ¹'@º'
ÛÑ"?ïîè¶7_¿ãDêJŒM¿ãI"â s¨¿à{ÿõï¿èiýà)¿ã,+6åo[AGNbll3FGL J0730.5-0537TXS 0728-054?ïøyÕƒT?KF}QÏmM?N«ò¬ÿ?KF}QÏm6?ïõËDîß?p•[+Ðjs?Tivx¢B¡?p•[+Ðjp?ïÔϋÒ#?v¾'>ki£?u˜:uîÝ?v¾'>ki¤?ïæ%±ýF?T§3¿öîü?iÚèN¹º?T§3¿öîò4FGL J0730.7-6602?Úàt¦*ÎÀ4ËݵR]À:(›)¼'ìÀ<Q7Âäì~@!>{ßI| ?û†×¥mã2?¸ûŽ^I·?§¯rÉÌf?ð$ύqm+@ó…'P¥¿ïäY`Äeö?ê$õî.Fd¿©7q@Ñƿޛ0þ$³"¿ÙXÜ¥‡äe¿Íóÿ*AGNbll3FGL J0730.5-6606PMN J0730-6602?ïùÒµ(?L OCÈ?KÿŒµ+_Þ?L OCÏ?ïü LC"n?Y>Z¥?>ýãd"™?Y>Z¢?ïÝñ€2sX?vLÍ^'—w?q?æÆT?vLÍ^'—|?ïÈáÙÍ?mº¥<#,?{qð¥?mº¥<#,4FGL J0731.2-1403¿éÚþ>"*6@–ù%ñ+QÀ:*Ógñ€áÀ;ʎo™ëÏ@ûL¶çÞ @/<c]j?п$ÃÍÕ?׈'=Y@·kcü(Û?ø›{HË Ó?âñn!›±!¿éçÇßþù¿Ü$ýŠ·¿ÞŠ0]¿î1ВT*ú¿ïùžrAGNbcuPMN J0731-1402?ؓG6¨?ËYTÇ~,H?ã¶z\d¬?ËYTÇ~,I?ÃãsBÌ?͒¢àªI§?ë#/\ÿ?͒¢àªI§?Ù)¨KWœ?¹hHVzO?ãxë+ÚT2?¹hHVzO?Ç'ªÀZ¢Ð?¦àDª(Q?ê6OéWK?¦àDª(Q4FGL J0731.8-3009?äuÙyŒï¸À–4T›bÇÀ:nb
·'À<'‰±Å@ n·Ã¦3@ʸ¥Î[B?ÃÝ
Ý~ Å?ÉÞ
¼×?Î*ÚÊ"Ý@åàÄüI¿å˪Þe{…¿ä¡L`«¼\¿Ø^ìŸ{¿èZa_ìNÈ¿Éŕ 
;¨¿è,¾|¨AGNbcu3FGL J0731.8-3010NVSS J073151-301058?ïõ‡¼)µÈ?Qß5ïNl?Tð‡¬"oL?Qß5ïN`?ïþ',#`?HÌ'…^Á?&Ý7
Éô‡?HÌ'…^È?ïÕîÝ?yk‡Ùu±l?uóy'y?yk‡Ùu±`?ïø£¸çÒf?AR"5±ÒX?Mq`¶eÅ?AR"5±ÒQ4FGL J0731.9+2805¿ë:®¤Ž@4¦£ßm¹AÀ;3x‰|ìÀ<·v Í|@ M«¤?þ{Ê`áÂ?Ю†ü#»?¼'îY?ìH^sRÝó@`¨܅ý¿ÕIÈ`u¿ë!ªªcy¿×ÖRß¾¿Óòó¨é¿âÒ;66ó²¿ïÿä¼­šØAGNbllRGB J0731+280?ïþ¬áJ¨¾?"®¨ÆæWI?%1ëUtê?"®¨ÆæW?ïûòñX´µ?]š"{!0›?@4:--g?]š"{!0©?ïì%Bʋ?hd ¸	¦?cÚ½<utÅ?hd ¸	°?ïè%oŠŠà?Q£…êî¦?gڐuu¥?Q£…êî®4FGL J0732.7-4638?·sr/‰a¼À)«"«CIÀ9ù±ñ\ÏÀ;·×Ñã@"ñ>q)ä@Õí6´È?ğUÆ0%?ß±Þ¿"~M@9½ÆŸŒ"@oÆÚðQ?ÙÉÉã
€ò¿Þ—$'¯À¿çXàÚö±¿íÞ[€px¿ïûE@Pýô¿ðAGNbcu3FGL J0732.2-4638PKS 0731-465?ïlyÑûÜ?šã)Cñº?'pÅÐ"W?šã)Cñº?ï¾vÑu\?ŸÞ'¦îÆ?€bK¹¢©?ŸÞ'¦îÆ?è.ڄ/ÀO?±kˆgEȖ?ÏD•ï@þÃ?±kˆgEȖ?î§Ü«2(?¯žJµ.?¥'5NœÝ'?¯žJµ-4FGL J0733.0+4915?琣üíÊb@:ÄÝ?á—_À;Ž"çƒ1xÀ<ÇÓØZ@ PÊwGà@¬Á¾¢h?ΐä>X€J?¦ƒÝ‰wQ?×ì$ÁUuR@ƒ,,®´´?ïÉ÷šÖ°{¿í',ˆG¿Ò–ñH­ü¿è]b
â¿×óµÄÈqs¿ß¤L%šAGNbcuTXS 0729+493?ïývÍèË¢?2ìILxÀ'?4I¹¢ê??2ìILx¿ô?ïþƘó'?RÙëbá?/ã–p͔·?RÙëbà?ïâÞqXR?s)͕u][?m!Žø§­þ?s)͕u]R?ïïÙÌãè?MñÌÛ­±?`&÷3ö?MñÌÛ­ª4FGL J0733.1+5910?æëª);o@@<KªX-¾À:¾åžTê=À<¼:ìe‰@£³1fª@Ûä—Å?‰Å!Ý ?½Ý¨<I²Q?ö-íy¾Ô?þ:|PªC?ï¹Ö…³2È¿à˜›¢ˆU¤¿á½Aԋ³¿å^ˆM@û¿è܄›Ó¤¿é ÷IíAGNbcu3FGL J0733.3+5904GB6 J0733+5909?ïŸÄ%ɗ? ^iðèm{?ŸL{FÍ? ^iðèm{?ïH3«qé?£AÊM'‹:?–ùŠ'ßé?£AÊM'‹:?îû©Þ7?–®ý·lÄ8? Enx¥?–®ý·lÄ4?ìÔ`Wÿ×Õ?%àqÏ?¹\ý@AX?%àqÏ4FGL J0733.4+5152¿ìW%)•ï@;PÜY1ÊÀ:œ˜¬3ÐÀ<'·I­Èü@ ëË|Àšå?üWu¸e?¾Ú¡ Ì~H?¤õg £#?éUM9n·@)Òh@Ž¿ë"Š.B¿á՚ }#¿ß½<:¨¿Ô;»P¿ã1Vº ù¿¾™AGNbcu3FGL J0733.5+5153NVSS J073326+515355?ïþ‡{«?"ŽÊÑÊip?'ˆOžFô?"ŽÊÑÊi´?ïþ·PK?G/´ûGÌú?/ďšûO©?G/´ûGÌå?ï÷Ÿ&œÕÈ?a禹=pq?PÁ²ÆTqS?a禹=py?ïíº,ÔY?QDòÜ —?bEÿÓ+©?QDòÜ š4FGL J0733.5-5445¿îz¦ÇʯÀ0-VJQ]À9àª_ºz»À<M‹^¿@ô¢""EB@?A^o!?·ÐK\tË?±š}Å'¼Ý?ø–ùáØ͌@j¼¨'Zá?ïûbví'¿ãŒdý°šg¿âdøbQÙ¼¿â/! 8B¿ãɵÁŒä¿ì"~w=AGNbcuSUMSS J073334-544544?ïÿyik?zêÎû©ð?ÒÝòÅ?zêÎû©|?ïýöØUÁ?Qj/¥‰Y
?0I=WyõÁ?Qj/¥‰Y?ïìkY‹¿]?l(|­¼"»?c"¦t@£×?l(|­¼"³?ïþ‹)ŽÀ?‡@mŒ·Y?'O
gô?‡@mŒ·Ù4FGL J0733.6+3649?ïñ‡—ó3@7ѾãÕýÎÀ:·óáäŒÀ<'³!*3@x\fˆJ<@°Ò€jôk?ÂÇ·#Ã(´?¨÷ð€ÊÚs?ã:¿ïn¸@
<åc?ï´èâÄ0¿ç+zl­¨D¿áֈ7q†U¿äx#'¬?¿íë¥jˆ4?ÑUÛ}¿žAGNbcuGB6 J0733+3650?ïùâ"ÉOý?Dw-ÃH¾W?Hu¬ÚÀS?Dw-ÃH¾L?ïý÷¿Úzá?J{Š;"ó>?0B,(ý¡?J{Š;"ó9?ï AK™¦L?ˆq»f/zÞ?‡ï­–mJ?ˆq»f/zÛ?ïö˜¥5?B07;Ö ^?Rεו×û?B07;Ö S4FGL J0733.7+0205c¿äýÎngÀU@$º±NÂóÀ:¬i—sN¬À<"/|@5@Í$¶n@è"C ç?ÑúeŒKÓ=?ϗ
Éĕ?÷›bÇuu@š1P/p?ޜJØw{?ïڍ¯ãˆ¿éÔ¿?E-¿äÙÇQbÉ#¿ëä¥Ï2¿ïÿú¡œGtAGNbcu4C +02.20 ?ì¾:ç¨?¹Ù<j.?º/? ÂÐ?¹Ù<j.?ìÐà›(5?ÃúAÍ
?¹yâû&¾U?ÃúAÍ
?èÑô"w¢?³zm0ƒCð?̸/uú!x?³zm0ƒCñ?ígª&È4~?¡þ5á
"}?´Â®É¾\?¡þ5á
"}4FGL J0733.7+4110¿Çù2Åܦ•@9
»ìª¸¦À:=~|Ý¡0À<yy1DEª@i%u°[R?þÙ.T§!B?ÀêÄ.˜™¿?ª€câAm?î]eÖômü@ݤ]ÂÓпØC¯AÌ~¿å5f͔s¿áˌ%<Ðk¿Ö®êäâ¿ØãP÷,r¿éUÂ@þAGNbll3FGL J0733.8+4108GB6 J0733+4111?ï÷¤µÎ´?DOÄÄÈk?Qʶ"b—M?DOÄÄÈh?ïþ ëT­L?DLë&Ñ?-ñJµ+/ý?DLë&Ï?ïèE·u²Ä?rr#Š¯™%?gºHŠM<?rr#Š¯™#?ïÓck?_‹8ù=$E?vyÎxpÊ;?_‹8ù=$B4FGL J0733.8+0455?îÍh"ëÏ@']—5;À9ÆØôù;ÁÀ<6	'_Á1@O}–®®@ÊZ¤'Da?º8vÿeÑ@?¾V§V›˜!@€ê[Sí@š˜jÅp¸?Å8(%
*¶¿å(Tf,Û¿äP‰OŸz"¿ä`
+Òì¡¿î`~oò¿ïÿâ~9ì¶AGNfsrqGB6 J0733+0456?ïúo.›Ø?TÀ¿"©©¥?FCçE ×?TÀ¿"©©«?ïúv¤$d&?f|Ö
—]{?F%onom9?f|Ö
—]z?ﬠ®š.\?"6°ë
$?"×ÔYthè?"6°ë
?ïýR"²9?$íQï†Td?5kÚn7?$íQï†Sõ4FGL J0734.0+5021¿ÕÙÒyù@;$"ƒ‡ß]À9áj'"À<gœâ#v'@ðy©åE@&ÜB‹•Ë?·ëp&É?Ä¥"¹¾R@5\FR@Àx¿¯Wò?ïÑ>¶ôô3¿×þT.U}á¿ç6òl¬Ò¿çÆžEÑ¿èX.•>Á¿ãò,"à`AGNfsrq3FGL J0733.8+5021TXS 0730+504?ïÐ÷¯÷h?sxeáqÝP?w"(Kþ ?sxeáqÝN?ïùš¢àQ?h´É>¿ió?I—¥t~¿|?h´É>¿iì?îðwQ(xè?"™xΡV? øŠíxq‡?"™xΡV?ïàï¥5T?Wñc-Kpc?oëZÊ«Ö?Wñc-Kpp4FGL J0734.4-7711?ïØ\üŽÀ8
à"S.À9i)•ûhÀ;ç$¿ÒéG@=@ޗz†@nXæK#?²§òø°€f?¾³k§ÃÓÕ@
í$%y6M@žL[Î2¿áÓ_
+¸¿ßM"ÜIm¿ã¤;é»¿ä ˜%ü¿éã{dû,\¿ïïÏ0T[¢AGNbcu3FGL J0734.3-7709PKS 0736-770?ïûÛ_¿'(?A®ÊxMjî?@'÷bZ?A®ÊxMjé?ïûÂ
Â.?[Ð/$}A?@÷ɼ÷MÊ?[Ð/$}=?ï\=ꄩ?ŽœS³ºðt?"xB¯jÞo?ŽœS³ºðq?ïýže*v?%8ÈC˜r'?3"Ö¬O`?%8ÈC˜ro4FGL J0737.3-8247?ïIqDÃ[ÛÀ9y¥CñÇXÀ9ڛ<1·À<8¸¤ Ü@ýäG'»¯?þ=þÈs¢?¶_l÷úøÚ?°ö!YìÛ`?ûz4ääÇ@9CiŒ5®¿ï£Ùqö½?ïÿxPsµÚ¿àý|Bם¿ÜS¿ð›^¿ÝĶv$J¿â°ÚÉÒ+AGNbcu3FGL J0737.8-8245SUMSS J073706-824836?ï÷W±'éµ?P©AìÈc?QPœÚ,–†?P©AìÈm?ïá$M?"ž4ÖÓ¤º?nó÷Û²þ;?"ž4ÖÓ¤º?ï³
üº³?'QZ⋽ð?ƒ<€Ñá?'QZ⋽ð?î×ó#5™V?'œ³|k»?¢€Í̦j£?'œ³|k¼4FGL J0738.1+1742?暣<½éà@2÷ß (À7@'§À:ÿ³"ý*c@[‡/‰°m?ÿ¬BÊ ?˜wñ†É?®îŸ&÷@Ý­àx{<@Õ r'B?É	¤C–­¬¿Ô<rwá¿á;ã:Í[h¿ßJål[¿âÔOb"Èõ¿ãY™~Á¦ÿAGNbll3FGL J0738.1+1741PKS 0735+17?ï÷ļÆò;?Küž î?Pv†rŠ?Küž ?ï³.ÆÛ¹ý? ¸~j4²&?ƒ4NI? ¸~j4²'?ïEàÙv'?Ž½ÅzGZU?‹î‡É¢uë?Ž½ÅzGZS?ïz¥!?†ù=bù.ç?Þp«[ë?†ù=bù.ç4FGL J0738.4+1539¿íê2X›
n@1O\žf‡ôÀ;mÄ@6PõÀ<½Üºí§@ °€¡¦‰?øT¨Ù ˜?Ø̙¡&V?âØ\î 0@t¤Ú¦@UîcöIž¿ïÄà\+¥?ٙiþX5?îŒÖ!à$˜¿Ò×ɓ\i¿æŽÏŒ0û¿ÖÃT¦Ë±AGNbcuNVSS J073824+153839?ïÄÇUg%?5Ià¤.?}ôœULm/?5Ià¤.?ïñúàËñ
?wÔ
çA?\
>hèn?wÔ
çA?ïlUFš}?‹˜^ŸCÏ%?'u_7,°A?‹˜^ŸCÏ+?ïF»;>]?…$ÙFt×=?—<˜˜4B?…$ÙFt×<4FGL J0739.2+0137¿ïE	ì9ö@&Á,I4&xÀ7')yv
£À;tcŠ	@¡œvmŀ@'>3Av?"[M¿·¡©?¸T=ë.H@ "¥Ξ@Wˆ"MÞ¿ÏòUk`K¿â³¼ÅîŒ:¿æL¢:Rf¿æ‰Ã}˜²¿ëÌ>1"÷¿æüÇ0«™vAGNfsrq3FGL J0739.4+0137PKS 0736+01?ïé–Ýû?`þo‡T	Í?fûi"<C«?`þo‡T	Ð?ïzù`è?¦Îƒ—`Õ{?‹áA§Åÿô?¦Îƒ—`Õz?ï]y¢v@?'M#€?Ë¡?"_P˱7÷?'M#€?Ë£?ïû|tšC?9h^¬N?B
ú-–ò÷?9h^¬(4FGL J0739.7+1743?ãÃØ 9@2qWÿ›V2À:˜)W_À;mÓÐÍŽ@å4`t	@ôZDïô?ÊÀDÔt?²ëJç.ù?ï+üÞ@âaFkõ¿Û0³¼…à¿éË4çhY†¿éôàM/¿Ý´áÙú2¿èìЮÝ*¿ïùÏdVÁ®AGNbcuNVSS J073948+174304?ïë;C8ó{?e	žZ»Æ?dļÇ"ü?e	žZ»Æ?ïóçËÚ	g?yA¦]Ä?X0hKí2?yA¦]Ä}?îÚØ>ë¦?žD¯¦ú	#?¦òR|Ež?žD¯¦ú	$?ïΟr¨?f)'׍'r?x°pF«ðÇ?f)'׍'z4FGL J0739.8-6722¿î!܌kØÀ4nÑáÃôÀ:døÄ¢[àÀ<[~ùc@ñØSŸ@ޝ"ÐÜý?µx…ø§ñ÷¿µ€°®ˆ"?ÿÜazn['@_"ØaV¿äw6b'œO¿åHþaur¿â÷<b|¿ã9wÑ¿ßØB·4µ¿áWß_¡{:AGNbcu1RXS J073928.1-672147?ïû÷¹Êê?8ÿ£õ°•Ç?@!×à[F?8ÿ£õ°•Û?ïþ…kM?=ªÓx‡Ðµ?'¯®YK?µ?=ªÓx‡Ð‰?ïنÃ$»?xæÔ"JG?s<žm¢}›?xæÔ"JD?ïûM-R?4 #±ŒŒ?CæËJµR?4 #±Œ 4FGL J0740.0-0753?êNÏò1@EàqÅ?:À:†_-À<ê°¢¦@µÏ‰?¯B@µj£	#?Ĕˆ7Çl'?¥ìã¼à?ß¿½WÓ|@P`ö:¿á
B[Ûs¿Ýbyýr-¿é±	ÝÏS¿é"ÛÈ¿í;'ô:Ïà?ã0} g(®AGNbcuPMN J0739-0747?ïã­;ó½	?sB_
eÿS?lRÄB÷"?sB_
eÿQ?ïöeèz
g?u€$ÉC^?S4/å2Ç?u€$ÉC^œ?ïx¢"Òx›?‹ß¥ƒT?ë­…°ì†?‹ß¥ƒQ?ïð­jr"?Oq•Æsj#?^¥+ñö-?Oq•Æsj14FGL J0740.4+7300¿èm*2^1@=l" ٔ[À:¼³ÑSDKÀ<;&Ö-Ÿ@}EÐïœ@
«£|qk?"f7.¢¿Å±KgŸV@øpž2@×´³Pz¿³·†
¢¿í^ܙÉjB¿éͽ"¨™¿À'Á¦Ss¿ìû2Ál"¿ïÿí@_Á‡AGNbcuNVSS J074111+725822?ïù[QMÙ?Xu7ïöÈ?J'»Æȝ™?Xu7ïöÈ?î8`suÍã?Á8OŽG?¬yøÈ£!Á?Á8OŽG?ï=`§­Œ?•ÂAàmì,?˜Së
OÎo?•ÂAàmì.?ï³<÷%y?öÎ	•´¾?ƒ0Â?¶¢?öÎ	•´¾4FGL J0740.9+3203?磴'ÅŠ@7Ϋ%(®À:®Ð!#~À<}æðdŠ@;Gxåo@¡ Ï?À<Ndçá¿ ž=ŠØ"?Þ®@dô÷8?÷úÚl1¿ªMìœöÆE¿å77¤±ü¿çÄóºw_³¿ØÒB­)¿ê0Bhv¿ìqýs]ÆAGNbllLEDA 1979979?ï¦Ó¤ß?|ŸÐ‰m~Ú?†K9Vøˆa?|ŸÐ‰m~à?ï`¦[›…?§MúÓփž?"ë4ŒœÏG?§MúÓփž?ï…ÂÅU£Â?…®«3גJ?ŽNª—Ï?…®«3גQ?î»Bw÷à?ªœ)Z–M?¤K؀ÿM?ªœ)Z–M4FGL J0741.0+3226?Ùðoõ®þ@7òu¸eÀ;̉>؂ãÀ<çH㞠@#/p-ºxa?õ1©u¯¯†?ÙVùvy!?ÔÅ:çÝt?üGZ·ÜzÀ@œ0K¿ï÷û^ۂ?î3;5t¬¿ïÿÿ^ðP`?ïÿþó…õ¿ÔŸÕÖÀ¿ÛÒ݈óAGNbllNVSS J074054+322600?ïéÔôm[¿?f˜Ë»?f+'¤@ò?f˜Ë»~?ïúà%HHU?gM±¿S?DjÞÞ©Ç?gM±¿S‰?¾)"?…Z]W-Æ`?ˆ:Pu·W?…Z]W-Æ`?ïïÜ4®‡1?\'þ&Sg?`#ËQxÏW?\'þ&Sg4FGL J0741.2-5140?쬋›Ö¯€À+Ÿ™€o&)À:oèuŸ¿NÀ;âŒÅuÀv@\ZôÃ6@™çZÌË?ÎÐè:fƒB?ȶUýb–Î?÷—'Ôà˜@±»ÚN¾?à;ÅþÒX}¿ÌÛybí`¿æàÍûü¿ëȬ¬›ÔÝ¿ïÿ$=Çâ?ïû…|¬#	AGNbcuPMN J0740-5137?ï¥_B'4f?¢)S.¾ù[?†¨/[ræm?¢)S.¾ùZ?ïeÓ!ª?¤ØÈkûd?"E›Ê¿ä?¤ØÈkûc?ë 
$•Ç?¬Kp1Gž?ÁËãm¨æ?¬Kp1Gž?ï\e.õ?Ž"NPeªe?Ÿ"sZ?áY?Ž"NPeªe4FGL J0741.4-4709¿ëü–r²'BÀ'zŒûüÀ:
O"'ÉœÀ;üýòÆ@	ýå¶@©EÄ/oY?Àw€bæÕ?¼íÜ
n?ø©¡Ñv@
Q©BO†?ëö@äv¸¿åð×~+©ý¿èF¬â¡ N¿ëä3¡<]¿é¾Îqèz¨?Ú/‰E
¦1AGNfsrqPMN J0741-4709?ïøãÐö?M"®'t?Np¼'ý?M"®'[?ïøºSI?rƒéÔø€?O³Âà*?rƒéÔø€?ï®Úø†}?ƒ»ùŸðā?"zÉAÞ`¾?ƒ»ùŸðÄ{?ïÙº…f"ý?ae"‰ú?s"½Lµ÷?ae"‰ú4FGL J0742.1+4902?ï`Ê¿"¹k@<0_¿ƒ8.À;7—Œy À<º%œq»@©†f‹û ?þ¼‡Tów\?Øj×DÁ?Øoâ+XÉ?ÿQßá|‡:@åµ{øI?æZà‹Ær@¿çÞÖÜH¿Ç&£"o8¿æóá^TI-¿ïûü€¿¿ïÿÅþ&ŒAGNfsrqGB6 J0742+4900?ïú‰¶v²Ê?IXW%üx?EÙ&%4܏?IXW%üx²?ïøE•yR?g""‹?Né«®»?g""ˆ?înc	H‹,?™ScÜö?©ÏkwM@?™ScÜö?ïa˜Jo?€ðš5ø?"Ìö¼ý²\?€ðš5ø4FGL J0742.6+5443?îykòz·@=øe×Ë.À8tÇåÝ?À;òc`øh\@š{ú!n»@Ê=p£×
?Šˆ¦úw¢?µª@8M@iæ@;Yr@üþËÍsf¿Ã§Íyps¿á¶vÛ)¿åÔþõhø¿ä_bцoñ¿éE¸põ6¿èŸ^ÕxlùAGNfsrq3FGL J0742.6+5444GB6 J0742+5444?ïúŸõ÷ÈÒ?@|>µ¢?E€( Ü»^?@|>µ¥?ïø"Zâ—?c4ƒ\3'Î?Owޔu¦V?c4ƒ\3'Ë?ïÜv@‰²Y?tSÉÕՁ?qÄß»&Ô<?tSÉÕÕ"?ïÿØæ&Wg>ëɤaóv_>óŒìÔLÍ&>ëɤaór–4FGL J0742.9-5242?¤ÒoùXæ0À,,©¬6TÀ:ê&yçMÀ;Ó·?œÎ@ÙqÍͨÀ@yÏ.´H?Åkøa%3ì?ӉU^?±@=X «Ó@òÿf}¿ï¯šAµ,?ï֘ȹAÖ¿ë+:¯(w¿ç±_ÞâÎí¿êzÇw"?׆·¿ŸgºAGNbcuPMN J0742-5241?î9"­ÇÞã?±{Ȅ7pY?¬gµ#'Ê?±{Ȅ7pY?î'*˜?À¤êBÙý?­Žž-VÜ?À¤êBÙü?éUN§W€?®49ÖW?Ê«–Åb¡þ?®49ÖW?î¬jaý?•È‡ƒš²†?¥9YîNO?•È‡ƒš²†4FGL J0743.0-5622?ÍÿÂåêGÀ/G™€o&)À:@NK½m´À<&¯söqâ@p|ЋU@w@GD?Äym>Ç»ì?Ãô¾""¥?úmlP‹3@"¿ÍŠâÈ?ïÍa¢‡Sò¿æ<|óp¥…¿ëDžj䥿åzÁҝÇ&¿çz4y"P¿ïÿþ½à ¿AGNfsrq3FGL J0742.6-5623PMN J0743-5619?ïüSý;§~?@o¯(Nƒv?=`"ÄÓ?@o¯(Nƒp?ïüZ@ÔIQ?]½º­‰?=-ù]µn?]½º­"?ïGU'Ýž?Žúf¨‡'q?—MÄL)?Žúf¨‡'l?ïã:ÅÝÒP?W¢ú>)=?lÅ:"-¯£?W¢ú>)?4FGL J0743.1+1713¿Ç;$™ÊÊ@2÷4Ö¡aåÀ:tt "ôÀ<UXª¼Í@îˆv܀@öQo^?À4X6ÍÇt?2¹ˆà?Ò
þ Vâ@"µW¿ìa>‰R¥?î'úC'œý¿ä£< oK½¿à}á,U¿Þ»ÎÍ®¿åëÐ}ÜNËAGNbllTXS 0740+173?ïÔ@üñHØ?rSù™?u߁‡["{?rSùš?ïúæ3?`¨q¾ð?Dgÿ3›¯'?`¨q¾ð?ïÌ Îèå³?|GRÕ@&?y'?|GRÕ@$?ïÒøEÉs{?eI¤Śv?vƒÝFC?eI¤Św4FGL J0743.3-4912c¿°²F1ã*À(ÌxB0üøÀ:Lâ\
WÀ<	_¨Ý|@®Ê_	Oà@¸E܃#6?Ŗ^%Ð;?À}Ãû
?ùÃk$;?îDæҝ~?íÌ:5…óÊ¿å{¦3Ûϟ¿è!æڕl¿èe¼ÝÁf½¿ã¢©][û©¿Øˆ§ƒè‡AGNbcu1FGL J0742.1-4849cMRC 0741-4900?ï™ÏÒÆ?'ï´ë±É?‰ŒNyM?'ï´ë±É?ê÷Àü¥?ËÖÉs7¿v?Ä#ˆÿè
e?ËÖÉs7¿v?î†ñd^×È?œ¡4ÅoD?§éºƒ€?œ¡4ÅoC?ßKù¼'À?·&w®ÛÁ?àZ!¾ø!?·&w®ÛÀ4FGL J0743.6-3805?àÆzX'£VÀNÁ;ŸÀ:A¨@üI'À;Èu2²ô@Ó .^7@¥Q]À¥w?È-Ûõ‰¯?¸[&þWÅu?ñۑ¦†'@__ô²D
¿Ø"€}¾Ç¦¿åOì!%êu¿åUŸ~àÛ¢¿å›û©Y*>¿égõèO	S¿ïü<@øî"AGNbcu3FGL J0744.1-3804PMN J0743-3804?ïûÎ,žU?9¹D‡b ?@ÇM…Š¥Š?9¹D‡b§?ïýå:Œ²}?VçòÕÊ'‹?0Ö+šlg?VçòÕÊ'?ï¥P'Õ@ù?ƒ*ªZÜ:'?†«ßJ¯ÁÇ?ƒ*ªZÜ:%?ïøjæíõ°?;'0"ác?NTdH)F&?;'0"á54FGL J0744.1+7434¿Û瘟Òl@='MÓØÀ:¾ù¥À<zŒþ€£ÿ@ –€
§Mâ?ÿ ¥&••ÿ?°¾ØmiåÍ¿ ‡ìa×OL?ðÂ0â (@7ÛÜ_;û?ç"5vÚQñ?d*®Ì©î¿åRÀâ]Ø£¿ÝB€Æ¿×1šânõ¿Í]v¾"eAGNbll3FGL J0744.3+7434MS 0737.9+7441?ïã
Œn³?d|L¾?lõs'=MX?d|LÀ?ïú'=Tç?]Lù%ùè@?Gc¶¬j±?]Lù%ùè9?ïÝðžm¾£?tàcìêç?q°É ®5?tàcìêá?µ¤=?w=y<ÐpÔ?ŽÛ'–ù°Ï?w=y<ÐpÓ4FGL J0744.2-6918?ÅølòÀ4ÇR"ÃÀ:'"Nü½À<E[sÄû@סçñÁ@œv"œ;?Ɨ–I­óï?°1,a¡Ÿf?æéHcF v@GÂWþÅ?ïû¬´('¿ÚZ[@B¿äü‹Rûпæå§#Å×æ¿éù>Dß-"¿ïóˆù8e¢AGNbcuPKS 0744-691?ïЊ
òž?vJïx­¯?wºùþ°½?vJïx­²?ïîu±Wl?wMR\º&?aŠìN¨•ß?wMR\º#?ï{B"–?"MÉ[bÍS?žP—­/?"MÉ[bÍU?³c´?sÔy,Ï)Ò?Ž<'Ý?sÔy,Ï)Ð4FGL J0745.4-2447¿âá¡°Ë¡§¿Ã<
ÍHÏÀ9¼1ˆ8HFÀ;]H2ž¹@¡Ž_S͈@ä4 ½?Ê>{eÒ?֋I?2É@¿)Æ¢ç @û
3\ó¿Ý9ÐÜ&$¿Ù†ðI©—>¿ìè®?Cî¿ê³¸þ¿ð?ï÷$ß³Y^AGNbcuPMN J0745-2451?îænUºå?©˜PqªKQ?¡™¯Q³?©˜PqªKQ?í™Y8ł?ÆD¢ÿ¢X@?·S569Óæ?ÆD¢ÿ¢X@?èþŠ	Ô4«?°ÖÒbœBr?Ì×د-P?°ÖÒbœBs?îDŒn¬[?œšù·—v?«·?‰:E?œšù·—u4FGL J0746.0-0039?ïð7j%¥Ó@'©Çy¦µÀ:¾?A^o!À<4Ÿá²7@4,}·eÝ@ûÙ_'F—?ʵ'ž}¯?‰Ú5b"ÑÙ?»æ'ølŽ?û÷-Uù†¿?ïÎúnƇ8¿ì	XÙµé[¿ì½ªðÙòO¿Í~(¤äÑP¿ïÊÿ'¬˜$¿ïÿ9+
ËAGNfsrqPKS 0743-006?ïóâ•Ù=?f&q\%`?Xü:ÔMˆé?f&q\%j?í˜Õ%
*?Ãٗ
[Sn?³9Vׯ¯?Ãٗ
[Sn?ï>Yø;i?–2O»l"?Ø4Àø'¾?–2O»l"?ï892,_Å?]…÷Ó?˜øÙºtW?]…÷Ó4FGL J0746.3-0225?KCù݉ÿ@&a·À9þoï|$>À<-Ý­sk@ fJ%3?ü<`Ÿ±?¼àC÷ü{f?³Á# k…_?ù×ÜEԉ@	VcȧN8¿ï‰\:­Ñ?ïÿñBÍÛ¿ä!¥Õèտϗ¯I.G;¿Õw•ì¼¿ä¾pžM³gAGNbll3FGL J0746.4-02252MASS J07462703-0225492?ïþžSP)a?&!!Å4{?&Êýið™?&!!Å4
?ïóAæ˞£?} Õ²8š?Y|2h¹·?} Õ²8˜?ïÖUœè?|73,î±?tóÕ81Œî?|73,î¶?ïðßëÕT?Mà!òPV?^@)ÞUV›?Mà!òPV4FGL J0746.4+2546?ï¤ïjÊB@6ފar
À9ºøW•KÀ<Ëùh6J@ó¿qÅj-@ýJ¡!?À2?WÙ°¶?П%ʔä(@	ÌDÑ	@ã$—9#¿ÖSb}£š¿åX&grÕà¿ìÅî Úk¿ìziR©ñ¿íeŠžT~¿ïý@'cAGNfsrq3FGL J0746.4+2540B2 0743+25?ïã/ã8Å?mJÂISQ9?lÐÇ<zÝ?mJÂISQ9?ïù=ªGlä?_È*B¢Âá?K	VâLjÁ?_È*B¢Âê?íPL@ßÕ?¢n;Ò݌?µ}ŸùI?¢n;Ò݋?ïìšÕüÌ¡?RÛ"õӋÁ?ce*3`(?RÛ"õӋË4FGL J0746.5+2730¿Ögn¦ ¹@7|.º'®›À:f…8¹"ñÀ<ZÛýÂ8@Wxð+̍@2³Ïà?È*2	h?Ï/՛'Ž9?øœ"ê-/ä@
»
±‰ÐN¿ä¿ôa¼2¡¿ÚPfíÖÞ¿ê
d1Xh¿ænd!¿ï­ÞA¿=¿ïã~õ©déAGNfsrqOI 272?ïuíôE@Z?'OyeÞìø?'BAwWôà?'OyeÞìø?ïý0@ª7Z?P
¹² ó?6}ú®E5¯?P
¹² ô?íÄ9ŠÑ(d? ]Œ¨xm?±Þ3©v¼à? ]Œ¨xm?ïîdD§S?Rm‰ƒw?a電X­?Rm‰ƒ‡4FGL J0746.5-0710?ì¤Íÿã`ž@! c¾ì9zÀ9ùÓ'é|À;úPA`ó`@µ¤ÝD"/@»;ªÐú?½_ÎÇ£Ã?ÊÛ¨‡É¤@V4êK@ÑâgÞª?¬MI£¦Ò¿â#BzMú¿Üt»(_šš¿àó 
Ì✿éÕùœ8°K¿ïÿÊ ¢¢WAGNbcu3FGL J0746.6-0706PMN J0746-0709?èŽÞDì&Ò?Â÷ˆôòå?ÍĆìOd»?Â÷ˆôòä?íYÓÍ}è+?Ã`qÝ_­?µ1a"¾§?Ã`qÝ_­?æ®~C!õ?ºÕ¸šÜYf?Ò£yͼ?ºÕ¸šÜYf?ì½zV"0Ã?…–L»Bñ?º-Kfyå?…–L»Bñ4FGL J0746.6-4754¿ê€ù`ŽÑ6À&œYyÀ9¾Ó-À;줾Éç@i*»ëS?ÿØIё?«Ý`\¥â?°ºž¡ì#@"8T~Ý@Ö2ÊÁ?íÐH¢†'L¿à‡·ïÅö¿àÂ_
§y¿Ýe¯¼ñv¿àUó‡K¹<¿ä®mє²ªAGNbll3FGL J0746.6-4756PMN J0746-4755?ïýøðÀ-?(Cå€Shê?0?Xyþ–9?(Cå€Shã?ïú|»8w?`ÅJzft?F
#Ë?`ÅJzft?ïåÖK÷¡?q<š¦ˆõ?j)´ì`V?q<š¦ˆõ?ïôXã;Þ?D1x³]²?WN9ˆCöœ?D1x³]¥4FGL J0747.2+4529¿æRr:©'@<hpdìé£À;8F:vôSÀ<½Hɝm@–•-NB?ü±'<ÓÅå?ÖÅi–œ?ÒAIvk—(?ýËûf=K»@O_™m¤É?îi* :8?ïÑÞïäÿÉ¿é¬ðžŽ ¿Ã`–‡f¿æ»E»Ëó‰¿ïù!bü$AGNbcuNVSS J074654+453231?ïä/Žúo3?nmµú]ü?kÐqËø?nmµú]ú?ïò—	[$(?p«EØÄ= ?ZÑíI·²/?p«EØÄ=!?ïvm$Hw?‰ó¤R·Â?'2[výÑ-?‰ó¤R·Ã?îÎ>3÷Õ0?'O7˜Í
?£À'¬â?'O7˜Í
4FGL J0747.3-3310¿ïüó€Ò‹ÀôÎf*…À8–·$¦À;J®ö"0¬@¦iÿÎÿ@"œî¸°?©cðüh,?zFäÚ¤j?ч-@´8"«ËË¿»ëXÔŸg¿Þ¡MÃqð¿æ¡wI¹L¿áÆy³JE¿åsUb2$?¿ç2¡<ü
AGNbll3FGL J0747.2-3311PKS 0745-330?ïû¾û—ˆ?=Wùؾ?A¡ùá+?=WùØá?ïþRŒÙþ¼?KÚóÛ ?*×2`;î?KÚóÛ?ï¬bá!VD?†B"BÛÐ6?"çG·ªo?†B"BÛÐ6?ïþÅÀ/'?ß*vy?#£ýFû®?ß*vy4FGL J0747.5+0905¿ë&#ÿ<ö@0zÝð,À:|]Îè0À<€ß©HcF@§e3‹rº@
Òä>š?½ëû€]—?¡ôsb€Ü<?æÃx?ô‡—5秿ï±×~¶ß?ïÿ´‰	)¿ân—²8Í¿âL^G³ó¸¿Üü³Ú¸rοÞüR@¿ÊAGNbll3FGL J0747.4+0904RX J0747.3+0905?ïí=˜øX?dÏd°¿ƒÂ?bàÂg¨q?dÏd°¿ƒÉ?&ˆ#?²ñìÕ%G?ïïû.û¨?²ñìÕ%G?ïµÜ(®¸s?€Y0[ÿš?'ˆõÔQâÜ?€Y0[ÿ™û?í9EÚïj?¢Ã(¤Û?¶5Ñ/脱?¢Ã(¤Û4FGL J0747.5-4927?ݵ¡`ü!À'ÑÀ¨ÒÁÀ:®rn²À< Ô¿ª¥@`Í p@ÍüŸù/+?ºšÒSÊW}?¦è©C¨Ù?ï˜ûC؜å@0Ûê÷Û¿àæäÀßXÁ¿ãQL=Æ4,¿æՒn,-…¿Þ¥€B/¥_¿ãì ¾üÕ¿éÙRKý."AGNbll3FGL J0747.5-49272MASS J07472476-4926332?ïï"ÖBs?Y3Œ¤ÝN?`{)½Œ~¾?Y3Œ¤ÝN?ïüÖsëiÎ?R&âú½|é?9L`¤±"z?R&âú½|å?ïãªâò#?tÜKîE?lU
Üç}?tÜKîL?ïω9³*?cH‹‰*C?x;tc&k[?cH‹‰*E4FGL J0748.0-1638¿Ã±zù´¶"@Ù½¥è\À9cÆOJÀ;´tÇR9‰@Ê·ÚwZU@LԁÌô:?¶iqž'óº?ÃnœÊPœ@xq¡šð@f'ÞdNß¿ÇûĜ|¢é¿å#—ŸC|¬¿é–ˆ¢ÑPÀ¿æŒ¹6£*¿îT6ž!¾—¿ïÚ¼i¨:AGNbcu3FGL J0748.0-1639TXS 0745-165?ïŠ~8P?@$ Œ?`\1ù,?@$ Œ?ï™ò"þÑÛ?£I
R.@w?‰ƒ^ÀK‰(?£I
R.@x?ï/7ҋ?'mM@ž?Ÿš™®Ð?'mM@?ï&£º³?'Pk¥ÝV?›+è¿Iª?'Pk¥ÝV4FGL J0748.3+8511¿êžPr3@<5‹¤
âÀ:´úȈšÀ<"çä€G¹@ ¶–*´Š?ø+®9cÎÜ?ÀOJ*›Š
?Ç
¸À¦@	ßøØK@ó÷ƒ¯¢p¿ïÿñ¢o+1?ïþ©ôZ°P?Î\u éY ¿ÐÐFŸ ¿à†é~3a¬¿×š¤ÆôE¸AGNbcu3FGL J0746.9+8511NVSS J074715+851208?ïìB
÷S¸?b"ù¿ä|Ä?c½ò¬Ge?b"ù¿ä|Á?ïô¤ÓÌw?lC?ŠŒ%?V¶YÆg0?lC?ŠŒ(?ïPK¾OAÆ?¯$e)…K?•öˆ6ÇS?¯$e)…L?ï^¹ïºŽ?~0L[}ñ;?"?(®t?~0L[}ñ>4FGL J0748.3+4928?ìóMï@@=AÿÅGÀ:µbÙéëÂÀ<Žn‰J—@€§i»Ûc@ü&V«Þ?ɝµÝòå?ÀçàúVGà?ö懈õÝg@²ê%MA|?ën0Ê£&á¿åÑ£€ùÊ¿ä¨ßá¿à–Fދ¼¿ï¼F¢{Àk¿ïZü¥Øl=AGNbll3FGL J0748.8+4929NVSS J074837+493040?ïï+"$?aN(þœ>?`ÔÝããÝk?aN(þœ:?ïü5õ¦"?V"kë?;–PRËa¤?V"kë!?ïÊ80u	?˼Ujr?zÿcçÅ{¸?˼Ujr?ï»Ê˜fv}?jY€®Ì®À?
Yæb`¹?jY€®Ì®¿4FGL J0748.6+2400¿Ð'·›z@6»³"ý*cÀ9T²ü(À<+%üéË
@ñ~Ý֊@S·RDÌ?²J¬azŠ?¯JŠ¹'B?÷ëýáAÏ@³a+"?áÓ¦¥ñ–±¿ä& !]ž¿ãÏâÌ'ª¿ã©&4G/i¿å'«_ê¡I¿ïÿþR€ÖTAGNfsrq3FGL J0748.3+2401OI 275?ïýîtMæŠ?.ãD¶/N:?0Œ]Ë¶¢?.ãD¶/MÈ?ïþ&Õ"Ìð?CÙ#[L?-'­Ó0çÓ?CÙ#[O?ïÜuø)Ú?vùv2ɪ`?qÅë}'?vùv2ɪW?ïþÑƳȌ?â}ä!T^?"ã"ÃwAú?â}ä!UC4FGL J0749.0-3904¿ç¨/¾ÉãÀ†?¼À:€ø¿™ÞcÀ;üFñ'@ 
=Šzò@+}\L1?È	<¿¤?²¯«~É^®?ícQÞïå?û½Ö½f}c¿ï`À¹n ?ïãÖ3}Ûοçxâ>ùæ¿ßøelkc%¿á}h@[9â¿ç
¢µ¢
ÜAGNbcuNVSS J074915-390336?ïê>ÉcÊ?b;¿Bä?eÁ6œp5á?b;¿BØ?ï­ÔÐ=B?¨¨ÑWèéy?"ŠËð»ï–?¨¨ÑWèéz?ïìó=Ð:?Š'dË`ÿ?Œ"Ã0‹ñ®?Š'dËa?î:Žc5ø:?™ƒE°î<?¬WÌ |n?™ƒE°î=4FGL J0749.0-2956?æݍ-é™À[íœP-?À:…ôÍzÀ;ނ€x`d@!$ÎÏÜKÆ@ŒÝÉtS?ÌÚväãÅ¿v«ÛKÑËË?ªŽ' cµ?øǟñøUg?؝¯]¦#k?Åíxé˶!¿Ü¤·$D
¿æ
š"U•^¿À7œ¨M¿ê¾;Ú¡¡¦AGNbcuNVSS J074913-295658?ï²<9¤"²?…fäOªŽI?ƒpñ–÷Sy?…fäOªŽG?ïÆùŸÏ-z?™Vº"4o?|ƒ0iBo?™Vº"4n?îᆯåÙ?•Ú@Xè$?¡î—•¢l?•Ú@Xè#?ï+¯µud?ŠÒs'è¡V?šŠ	Q_"W?ŠÒs'è¡U4FGL J0749.2+2314¿ì‰Ùö°[p@6–Κ,fÀ;˜+ÛPÀ<ÖÖ@ ÚêYûsÿ?ÿJ¹t*t?Ä#ÛýA^Å¿"=Ý8ÞKƒ?ÑÚ@þ¢Ý»?úñ¡µòÀ§?í8"ñœî?ÕHÒ¡ø㬿æq®ÞÐ/ƒ¿Üå<hš¿àO×äXÍ¿Ðq‡+ØÌAGNbllRX J0749.2+2313?ïõ9ûU)d?Q©M¼Pk?UŒ	U­7Ü?Q©M¼Pp?ïåïøµMh?–rvÚ3µ?jJ²™?–rvÚ3¶?ïëØ˲.ù?gŸTŸs6?d'4MÑ›?gŸTŸsJ?ï@XñL˜?'öh(96?—ôþ!Öm?'öh(974FGL J0749.3+4453¿Œ>å—@\@<¨1zÌNùÀ9ݍƒá¡pÀ<sn]«¬Â@"'Êö@o¡—Zû?µºµ|Ô?À0µS^w@c<æ:\@
щ5ô-º?ïèB©È»Æ¿Ý꣢\
î¿ãÔÖáΑž¿ä†J!aN¤¿è ÈÝ~ö«¿ï÷½ ‡_AGNbcu3FGL J0749.0+4459SDSS J074916.88+445232.1?ïꬃÖøN?cÖoènL?eS|)±Û?cÖoènZ?ïø'õå?cÜy£ÓÞ?M»°+àmì?cÜy£ÓÞ?ýŠ
?ˆI¢rI?À|¹Ù?ˆI¢rK?ﭒÑ-ËL?jõoòiÚÍ?"›K´,¤?jõoòiÚÏ4FGL J0749.4+1058¿á%¶¥OX@1Î=ÁçÀ:*GÒ&©À<J.oL@Xž¸ge@ø¨ê'?¸?W?JÂ?wâ?Âç?ÃÓ8KËÛ@¤©Ü‡ÕÍ¿Ñt
~^)׿ç¼Ä¬lÚõ¿çi'"š\¿Û/[ßyοæÀÒ@Ìú¿åâ,EhAGNbcu3FGL J0749.4+1059TXS 0746+110?ïã13¾¢"?iÊ»\_(?lÎÌA]n(?iÊ»\_(?ïü}"µt•?\©^Ä'Û?<ZT[W¡?\©^Ä'Î?ïÌnÛÜ,?{ÚØÄM?yȒéóY?{ÚØÄM?ïèU©)'?SÕlôß?gªVÖmà‹?SÕlôß4FGL J0749.6+1324?ïŽkby¼-@2ÝËݹ"À:űg¸ÏÀ<uTZË'±@·‹òçê?ÿb¡e?õ¹?Ð@gä•ÁH?àsNÁ¯r@v&}BJþ@Sò•í=¿â·îÿQ¯J¿Ý§!ïi¿Òo,Åǿ敏~¤™¿ïûæàõ"׿ãJ½É#ÊàAGNbcu3FGL J0749.5+1320SDSS J074935.95+132156.0?å8ž	i²?˼æ[Ü?ՎÃí-àœ?˼æ[Ü?á7GXy'ÿ?ÔÆ®µ1Es?ݑqOÚ?ÔÆ®µ1Es?Ò°hñró†?»$*ùa¸?æ§Ë‡F†=?»$*ùa·?åÉHæï,?´"fßý?ÔmÙn2!©?´"fßý4FGL J0749.7+7450¿¹öΗÉ¡@=éSXl¨ À:ð‹+AÍÀ<³ çTº@ )'_
ž@N~:˜'B?½ÿ ‡	7¿®"ä¼é¼?ïñà'Œ7@ël‡è—.¿á!‡Ջ¿ì·¬ª–¿Íõ:ꌦA¿ä¬©áæ9…¿ÐîqãD"¿ê݃¬8XAGNbllRX J0749.4+7451?ïù8äÄ^¶?Eä´ùO Ä?Klî…(ª?Eä´ùO ¹?ïþ‹F,Ç]?Cœ	(‰|?'K3Š(ë?Cœ	(‰e?ïáŒÍ«Ò?y'Rä°ž?nsé2T.t?y'Rä°£?ïñ7}–1?JSäkP1?]'Óӝn?JSäkPX4FGL J0749.9+1823?ѝÌ('ù@4ëßÁœ"À:eËΠ¤À<ÑEØQe@w–÷Cï@ÀXeã‹?ÂáðöLÍä?¯5z`Cb?êæEy†Ô›@	7>$þ½
?ïýU–4ŠK¿èž¿=˜¿ß×µž‡êð¿ì0¯?ž%š¿Î?|í'hs¿ïÿÞ˜–dAGNfsrqTXS 0747+185?ïýå»&Öì?7KÉHy?0Ò&ÉHÃ?7KÉHy?ïü½úC•?^@x{'â…?:-ãW?^@x{'âv?ïÁ×æS_u?{ÝÝg­7O?ÖPE¸?{ÝÝg­7W?ïùž^@'?<ùÆ,3Æ?I‡¶†ý÷€?<ùÆ,3°4FGL J0750.8+1229?åŽÀžv@@2¼… ¾Q	À9g¥‡À<E8ï4×@à–ºìûk@äǕU?°Â5o"¢—?³K—ƒñ$@"ºkáÐ@.Ó8¡²?î¡À_@˜¿âDÞ¥gX¿èŸJrÉK¿ãÂð	è·¿ëÌùÆ·à¿Ü¨ÿéåAGNfsrq3FGL J0750.6+1232OI 280?ïø…Â'YÞ?CòïcQK"?Mè÷b˜‡&?CòïcQK†?ïúμaÅP?[†­8Z²
?DÅxêºj?[†­8Z²?ï¸à«ì¼?{rï)Ûß?üÇÕÑ=?{rï)ÛÝ?ïü¦8®?+‰¸êûE?:Î?'â',?+‰¸êúÕ4FGL J0751.0+7908¿ïÜÅWyŠÍ@=gT~–À:ŽàùÀ<ƒØž'&ß@n"ˆ7Ç?ÿŽÑõ*¹è?¹.fDØw%?ÊOʘ•Â@ m֝0'@t—>u†•?ÈA•Ì…0¿Ê³!€nÅ¿á	}±Ç¿âÌËN¿ëB‰Œ¿çŽd²1@AGNbcu3FGL J0748.5+7910JVAS J0750+7909?ï!v~é?œÌãºZ`?Ÿ{Ñ0<ä?œÌãºZ`!?ïøò×lZ?h][ë*¬A?L7"¢N"
?h][ë*¬??æôØ9ȼæ?²RÎ^érv?ÒOŒn†4?²RÎ^érv?ïö¯-+¢?=boB?R¡¥©àºÑ?=boB-4FGL J0751.0-5131?ßå,·às¢À(Ç\¢˜FÀ9‹B¾ÁqÀ;µgôÛߏ@ÅûI{@mÆâ¨e?®Ðó"!?ÄrlN'@Dä]ã
&@ØP¹€ë¿Ò7¡¢&°ï¿ÝÌÔ#Ù#¿æ§¾ aŸ¿å`Âl »¿é™QÀg
Ö¿ðAGNbcuPMN J0751-5134?ïîŔ×8•?[½wý¼?a:k(Çjì?[½wý»?ïûÉy
·L?T²W'
ºÎ?@ÚÉ"Ôr?T²W'
ºÔ?ï±ÂÙQ–?–:x±Za?Ÿ©Ç¤ÕÍ&?–:x±Za?ïÿE$Á°É?
P†¶·Ù?[gÉæÜ©?
P†¶·K4FGL J0751.4-0421¿æáÛ4½j@&¨?NÊhÀ:v6¾/À<k;÷'@k•\É¿?ü5g‹)"N?ÐKÚ®?ÑjÇôö·'@£øôõ
?ôr!èÝúr¿ã™µž2µ¿á1†:A¿Ôy_ã•f¿Ùýh
«T­¿ãí˜>¥­#¿ïÿêњ'çAGNbcuPMN J0751-0421?ïǶ±U›H?"C·¢ç?|$§U2\˜?"C·¢ç?ëXìX?ÉdpvEÕ?ÃޜO¦Ÿì?ÉdpvEÕ?í°¥Y~T†?¤ÔŠ—õÄ?²zÕ4
[ß?¤ÔŠ—õÃ?èä.$;rU?ªíþlt?ÌoGo6«?ªíþlt4FGL J0751.4+2655?ã\TDÝg@8Tòù‡@À;fØ9¦ëÀ<ÍcЉð¯@; Ákš®?þ'¨¸]ª?ÔÙÄ❙ƒ?ہ¬]@¢Ý@Õ™Qu>@¾ù:!E¿ÕêÔà«"?Î9íwYo?¦dƒ7W…¿àÏûÀÖ…¿æ¨Zý|˜¿ïûC½Äò
AGNbcuMG2 J075139+2657?ïõ#´Õ?Q˜úÕŠ%?U¹ô–Uä'?Q˜úÕŠ ?ïùñvòã²?eHډ	Ñ"?H:$4q35?eHډ	Ñ#?ïJ7â!
?·e
×T?–¹»Þ­û?·e
×S?À_?pë´ C?‰W¹Ûè)?pë´ B4FGL J0752.2+3313?ÕÝ]YoZm@:lʁ˜ñÔÀ8÷tü+_)À<O²ÅºŠ@ùãÏrÄn@xô›Gïƒ?§-€Ä$v?¾}p@é@ˆIDíoÛ@ |ò–?¬9¥=;ʱ¿â?"À´W¿æFñ¡B…a¿æ"ύd¿ì@9
ãˆÑ¿å›«–òAGNfsrqOI 380?ïóõškX†?Skv'ˆu'?XË)NõÞ?Skv'ˆu~?ïúXàÙH?_XeÉ"?Fœ|›'ÞN?_XeÉv?ïžþL«ˆË?†–ùëIJ(?ˆ@lÕÍ:?†–ùëIJ&?ïÿð×>ÖøF±nâ4>ÞåÎÞQÏ>ÖøF±nèè4FGL J0752.3-1631¿áÜ©"Ðñ@«Oag#%À9ÕVÅßrÂÀ< szK@ #@vè•?þ&ƒøG¥?¼ºD^ÿ"Ë?Á̈ĵ&=@ucߣi&?ú"®LˆÅ?ï…þ|rAf?äl{‰
Z\¿Ú,̼±¡£¿Õ»m߁…Q¿æÎ[}Õ¿×*Šbo
ûAGNbcu3FGL J0752.6-1629NVSS J075223-163340?î·Ëo¿=?žèš™€Ô²?¤ƒI.}?žèš™€Ô²?Ü5×QtH?Ôè¡lcV?áårWEÝ?Ôè¡lcV?îgŽ´®¼É?Ÿz®â`Þ?©‡µ3r?Ÿz®â`Þ?ßâÌÊ?µ—ÛÜ9'?àŽ™šõý?µ—ÛÜ9'4FGL J0753.0+5353?å˜TäLb@>8Go*ZÀ9
Ó	ý¯ÄÀ<:wÓv4:@åø˃K¤@±Èd?¥*.B؏?©× –V!@ÕY;¸Ì@o¥åW]4?í¿ÂWþė¿Ü³_=}9¿â¶2÷¤ì¿ß‡¼Aº4š¿æ¸¸
"'r¿â}i[
AGNbll3FGL J0753.1+53534C +54.15?ïސO­"?qQˆå§`§?p·ðØ)>`?qQˆå§`¨?îùOõÔÞ?¸nÓd¢ª? k¢¾Â&?¸nÓd¢ª?ï¼QR?'È10Þ#?€ë¿ü+}9?'È10Þ$?ìÈïÔòԉ?¤K‰ÔÈöÝ?¹¸Xi[µ?¤K‰ÔÈöÝ4FGL J0753.9+0923¿áTyíÝÐ7@2g,®À:Õ±°ç"À<ZzyBáý@½sO­è0@¶¾`"‡?ÈïèÛ¡&?Ô¼K?™s@>¼ž_ç@h	S»¿?ïýCÂÍoŠ¿â'‰¢€õ¿âzSƒ4Ó¿åùP¹Uø¿ïÿþÐñ?í–Ö;
˜	AGNbcuTXS 0751+095?ïÚÁRŒû?xV°:ë¹m?rŸV¹'9'?xV°:ë¹k?ïÚM(h2?•îmzS?rÙkËæðê?•îmzR?ì&oéú?Q?¦?ÄbBVé?¾Ì€°.x?¦?ÄbBVè?ï³yözõƒ?sWxTêF?ƒ!'aBŸl?sWxTêE4FGL J0754.0+0451¿àáöjaž)@0$ã—­À:|­""aTÀ<~Ç¡é@ÔÈÜÓ*4?ü(æÞÆÊT?Ææ¾ûÓËo?Ç­œZêo@Wþßn@RbÊÐs?ïà&±D±
¿ÑiòâáH¿Õ'-ks¡¿Ñ´Î¾¿mê¿áarŒÖ¿æêB^IasAGNbcuGB6 J0754+0452?ïí¤Ôú†*?fTÍì5æ1?b[+y×?fTÍì5æ4?ïò'´]t?z\
­;!?ZܖÅEž?z\
­;!?ï°
ꉲ?ƒšÛ¯Xy?ƒÿ|…]"†?ƒšÛ¯Xy?ïš'jáa?kìu¨[z
?‰v%Gºgß?kìu¨[z4FGL J0754.4-1148¿ÀôÂÓc?Ú@ w9°$öZÀ8À"Ú›§À;­c¤G@êìž#l@?¶~¬®I?¥â‡ÁwP'?¶×ÉU"@ÅÐãe–@	û?ˆ??ãÕ6":¿×æÎÁ¹Š¿ãR­·]Ï¿¿á¡'bD˜¶¿àkö"o³í¿ìGÊϜŠæAGNbll3FGL J0754.4-1148TXS 0752-116?ïË2kߤË?}S¡Vßb"?zfÊ-™À?}S¡Vßb ?îÝÆÓVP?´¡c':cf?¢#'Î
šê?´¡c':cf?îÛK:
u?™.êÝ+"?¢KL^¯(£?™.êÝ+ƒ?íFÁDZ[B?•âǎcB?µÉñÂu%ô?•âǎcB4FGL J0754.7+4823?㩔¥³FÖ@>%–À8þáv§ý
À;æêð¤Bj@ào
¤É£?ÿ¸lrïá¥?§Ÿ!Ìa ?¶	8ãÌB¹@Ûwb7,½@P°ò{³¿áM¶ígw¿Ý;$-ܲ¿áQ"'›¿ßbÓ^â8š¿ç—'¾
è¿ç½w>û¾RAGNbll3FGL J0754.8+4824GB1 0751+485?ïýôgØé·?,+˜ÉîÁD?0\Á8²=)?,+˜ÉîÀì?ïøtl ‡?`a|ËUÊ?N.O}㔽?`a|ËUÊ
?ﺜÕÒY?†‰B§m?Xʾ‹iu?†‰B§r?ïêŽ?YWÌ?Qð¯ž(ǎ?eqÀ¦¨4ø?Qð¯ž(Ǘ4FGL J0756.3-6431?æüً7CzÀ1¼¡œZÀ:֞©£ÒØÀ< ö¼Š@ Š›QT±]@´¨+-?Çù¸¢ž?;1%ß/?»hø=¾Ò@€?Œ‡ã9?ï•[¬£7¿æe"®£¿Ìw3=D.-¿ãE=¼h|¿àgAøÈÔ¿ÓK‡½ÏAGNbll3FGL J0756.3-6433SUMSS J075625-643031?ïú`…'"?AIüDÎÕ,?E¾}é»{?AIüDÎÕ:?ïþ'^Ó¶P?IÕ
Vzú?-ŠĚÿ?IÕ
Vzù?ïìR¿9	?o³÷="?cÿ­@Æø•?o³÷=x?ïßY.A"Ú?Zm(=¨D?pShß5"
?Zm(=¨D	4FGL J0757.1-3729¿ÑJU÷ûsNÀß}úâ~À:­"àòôÀ< F.¸z/@"æìސ?ûV¯TÊ?Íá c6?ȄiF?ªe?ü¯©öÞï@ìIŸSÃ?âSˆ¾*´¿ïÆ~ŸBP?ïÿú÷''ý¿ÙiÉ<Ÿm™¿×c(ƒ×»h¿Û`~oòAGNbllNVSS J075714-372734?ï÷Aǐ[Y?VQß=ú?Q|pßIL÷?VQß=þ?ïýð†'?JΙ!õm«?0{ÏoÆÐß?JΙ!õm³?ï«'â½Ö?…âЇàïÒ?…6PŠyÛ?…âЇàïÒ?ïÏõÂZ?mb—©JÒ²?xðñÒÔ?mb—©JÒ»4FGL J0757.1+0956¿åÅ&³"@3Ø{V¸À8¾Ø»™À;ëùŒHx@
Òw[¬#@ý¶ÿÛíÒ?¤™,v«®?£Ï@ ?þçp6ÉÀ©@"®%lÌ¿ÄÙn[Ra!¿ß$ÑÜFw¿ã<æÀ"Ùf¿â¥ôñ¯e¿åC5ªøh¿Öß³#®ZòAGNbll3FGL J0757.0+0956PKS 0754+100?ïõd¨ì$Û?Q"Ãj?U6®'¶KU?Q"Ãf?ïîêçͺœ?{^^!Uû?a2Ed(?{^^!Uú?ïÐڌØÄ?ZéÈ~Ï?w'¹"òx?ZéÈ~Í?﵍Ï(y?qEåØe{?'œŒ5á¾?qEåØe{4FGL J0758.1+1134¿êë¸Ó0@3ú\å´$_À:ŸÒ¡"$À<}၏·™@ˆßµ\Ã¥@úz¡'¶?Àñ'êRï'?¥B#ªÃÒ?å†Å&6@#¹˜'‰?›v«Ô¿äQ›2öÍQ¿ç7"+#¿ÜWGd˜…ó¿æ¨î#;n¿âLÜõ)AGNfsrq3FGL J0758.1+1130TXS 0755+117?ïóÒ<¨¡?Xéˆ%‰Ãî?X[†®¼æ?Xéˆ%‰Ãò?ïû‡úsª?[3!	È?Aã¸1U™?[3!	È?ïòË|#ô"?g´GÒë?Zi¸÷.?g´GÒâ?ïìMÖgã?L»Kk"?c²)˜ñý?L»Kky4FGL J0758.7+3746?ì?¡3ÞêT@<áµ ÝDÀ;+"7ÉÀ<³bØ<l˜@\lû+@èy=Ùc?ÏBH¤ßrí?´~<Pé'?å÷SSd+#?ýœ"Áéð¿ï,æ}wúã?ï¬{­¿ÑPÜÚ¿Ö!yÍKwο꫇½Ï¿ÅoU®2XAGNrdg3FGL J0758.7+3747NGC 2484?ïë¶&Yë?`z£H%3?dIÙ¦ù|?`z£H%3?ï㌢uÓ?ŽmÂJŽ?ls]Šb.?ŽmÂJŽ?ï@…¼´Mk?æ¦ð?—ïHivR·?æ¦ð?ïh¥{œ?¡·±I"?'ýëP‡¬y?¡·±I"4FGL J0758.9+2703?ìÚé—@9ðr° ĜÀ9òÛª¶"À<mžƒä%¯@R­²«8}@Òáüߺ?¶'›}>o?ª°CÃèçN?ñï
D& ~@yıJe¿Ýpä+Ž#¿àJ¾ëÔ¿ãÑ.[]¿Ýó‹=
w}¿å'6É?¿è7fhê¥%AGNbll3FGL J0758.9+2705SDSS J075846.99+270515.5?ïé6¼?aw»a£?fɀ€CèÂ?aw»a¢?ïù½Ñ›^}?b¡JeáW?I¹'†3?b¡JeáX?ïÌÌ»¤?z֗ÁÅ(à?y™ø¢|.?z֗ÁÅ(Ý?ïŸJß(?s0*%ß½Ô?ˆ-[È?öL?s0*%ß½Ó4FGL J0759.6+1321?âü-[F»@5dàTiÀ:l¸ÿÀ<eä«æ£8@!K€0¼á?ú™C¬Äð?Åޒ\ŽvP?»«w¯?÷)sçXiN@®¡úçr?ï'h@Žf¿î˜›Ø8:Ú?ä^C¯'9¿ÝʢԀ˿Ãn9ÙënN¿äyT¼AGNbllSDSS J075936.13+132117.8?ïÿH@ }?Îó'«D?ÿ÷ëðm­?Îó'«D.?ïý5
Œ×Ý?P}®Îήn?6W"™A£?P}®Îή?ïùqát7n?`²Úµ?J8z/"N>?`²Ú²?ïòê˜ÆÊS?Nµ'›â?Z*Îrk]`?Nµ'›í4FGL J0800.3+5611¿É?'Çͨì@?³df±æÀ;:V=#wÀ<ÐÍ;‡•‹@ ­%èqï?þJå†×õö?Çy €"?Áþ"ÅõB?øÛkEÉ7í@;‹Œ:¶_?ï¬)¿*å¿Ø±ÁQ™{¿çýÀTïEž?î"ó—'Ø¿å€ê«Ú便åŒXž&ÇAGNbcu1RXS J080017.3+561116?ïôq±Ý¹?UªRIÊW	?WœDŽ?UªRIÊVñ?ïû¯"Ù?[Ĩ,c ø?ACÇ­ì›ü?[Ĩ,c ù?ïáñQ)÷?t÷÷Öû¾?n®Öo	€?t÷÷Öû±?ï¡-b†kò?pÝÖì߅?‡´§^e|?pÝÖì߈4FGL J0800.4-2257¿ç–ÿ"7ü@
戢ÑPÀÀ:L1ž½dÀ<S±Wü@@*°,Øü@…/‡­?ōi(dM?ÙÁZ]™Ž1@w¡øì@`[ÁqÏÑ?æŽMÀÓm?ÀÂQÔÒ*¿äé¾4ù‡¿åîoês¦Á¿ïÿñ7n+¿Ù¼®;è
›AGNbcuPMN J0800-2302?Ø~ÓºñÜ?ÊÉsÌ*?ãÀ–"‡8?ÊÉsÌ*?åã:¬R$?Õ3z؊³¯?Ô9Š§[·ô?Õ3z؊³¯?Øm'œ$?¶éÉ›:?ãÉp971ï?¶éÉ›9?è¥îqt?ªžÆ}—ô?ÍhF;»Ò1?ªžÆ}—ô4FGL J0800.9+4401?ï"צà"I@>‰ˆÁÛCÀ:Y:ßÏÞÐÀ<ŸOœ†@'ä¦èb@\ºÞ¿q?ÀuF©Éô?ÁGwÖø@1œZ>:@
åÜæuje¿ë¾«Â0O¿À*lD̹¿â¼,5èð¿â$!È`¿åeˆ…ug¿êœÞ|w AGNbll3FGL J0800.9+4401B3 0757+441?ïüÖ'´Ø?=Ìz:ɏx?9OÆÂYH¯?=Ìz:ɏ­?ïýbSû"?MvËA9vÃ?4í`&ïë¶?MvËA9vÏ?ïÚoŠƒëù?u¥lss¿@?rÈ:¾
1?u¥lss¿C?ïõ>ÙKmù?C|€|0?U'Mi$ ?C|€|0y4FGL J0801.1+1335?äeˆˆxK@5yj&åGÀ;UDêÜ0À<˜'6ôˆÓ@GCeÛQ@oå]½Jy?Ï_×@™"P?®3‰ð.PË?â{wN:@M€VQ›S?êم!½j?à-‰Àނ¿ì\Þþ'¹¿¾_g¥«¡¿év±'n"ÿïÿûbâMhAGNbllNVSS J080115+133643?ïÏXFxS?y¿þ^'t?xSÜÃÖ}Þ?y¿þ^'q?ï¯"uށ?œpÔB`?"<"ˆ_È?œpÔBa?ïM6Då9=?ŽÁ¹ä^‹?–Y7cXØ[?ŽÁ¹ä^ˆ?ïSö1$0<?'Ëö‹–?•9Ûyøo?'Ëö‹–4FGL J0801.1+6444?ç¼K@oæó@?¿#FV%§À:ܯæ8óÀ<ͼª R@ïÛ›l@^	Zõ?ÀQמ?Ž_^E–ÉA?Ð(€ý–nA@±ýx¼)g?Òdè'4ù¿å|, oa7¿ä& Z¾h¿Ú•ï ·E&¿á?›÷Aë]¿àLÜ¢,æAGNbllRX J0801.0+6444?ïþíðø6Ï?Tၧ¹ï?! ð|""?Tၧ¹í?ïþ4è?D
àuQ ?,±—.e§?D
àuQu?ïü³¯Ï¿Â?Sð¿bÞÜX?:b'ó3?Sð¿bÞÜG?ïþ?Ò6͸?6µ¨F?,ܓ$r'?6µ¨Ï4FGL J0801.3+6631?Ê3XJò±G@?¥yžQ?À:Ö§"þÀ<£dύqm@î8­Ež@©¸ËŽ?Ë{«r	1Ø?ɔçÙ³Ñ?öl×[œ@¨»R¦ëè?é'ôÛߏG¿â̎\X¿é¦Ê;"¿âa‹¶'¿é–lˆ¿Vÿïþí{˜ý'AGNbcuGB6 J0801+6639?ïrJ"í?•['»øc?'¶¼¢_ê?•['»øc?ïõv"2o@?vü²ÓO€1?U÷›!€è?vü²ÓO€3?î*:É:§™?Ÿ3t	ëŠ?­\SlU†Y?Ÿ3t	ë…?ïoúé?xà׍H&?'¢Â/Ž‡?xà׍H&4FGL J0802.0+1006¿ÖXÈז1@491"·ºíÀ:€®@ð‹À<zÛmy€@Ÿ*Þzõ?ÿM"þ1ɧ?Á#ÖÉÐÃý?¼)m↝?üI¬|]?ûÌpk¢æI¿î1ºÂß
A?ÖW•}«&Š¿à C=¿Û|ÂHds¿ä+"Xœ‰¿âr¼Jž‰ÃAGNbll3FGL J0802.0+1005NVSS J080159+100535?ïæsT3?k«R4i??iŒ«âãÌu?k«R4i? ?ï+j§sS?²X¡(ñ܏?š'¾•"?²X¡(ñ܎?ïÏK¯d ?xy³¨SÔ?xZ(xÍ°X?xy³¨SÌ?í?(×v¥x?™òéˆú.À?¶¹DJÔG?™òéˆú.Á4FGL J0802.3-0942¿êi\M]@%çÄÁe~À9Ï6¿yÀ<#Ÿ¢È…@ 0ÊڄEt?ýî%\°Úÿ?¸ƒ|-""?¦Öñ`Lh[?ñ7¼šO¡ÿ@œ•.ûÁ¿ÕTúe
¿è‹Ëz½5€¿ÞßeUÅ¿Ù8I½¹3"¿ØϹü‰Ð¿æŠQýù•ƒAGNbcu3FGL J0802.3-0941WISEA J080215.63-094250.9?ïû~¤ï?:Lÿƒ@½?Bo¥øFÇ?:Lÿƒ@²?ïúwbµßò?`£—8—h?F"u(€2?`£—8—g?ïðÅ¿W?bˆéOzcH?^uQÜ?bˆéOzc=?ï熬R-•?UR0_?›"?hyS­Òjv?UR0_?›Ž4FGL J0803.0+2439¿çŽ'iÝ¿@:»'ˆÛÀ;o"1zÌÀ<ºëªÞe|@ á:á}]ú@¢(ÁÀ)P?ÂX\›D¿¶YXê?ð·…Ýúòz@ýµ\Í¿":B¤â1¿âùóv"Á›¿äï:€.Ž‰¿í
DVq%Ý?܌%þpÛ¿Á
ôeB$AGNbllNVSS J080307+243749?ïú,ÿ,å?FÅr†=Ó?GLLk'¹?FÅr†=Ù?ïþ*s»À?FКv…Ä?-XÎÄCñA?FКv…Ãê?ïØz<å?{Q¤ƒk"Í?sÂûá÷Ž3?{Q¤ƒk"Í?ïý!r«5Ò?2{	?6ôj¦Qx<?2{Ù4FGL J0803.2-0337?r_!.ÑI@,b€àe0À9<IðuÀ<3{W3@=ÚÞ]mï?ÿ×¾³.–?ªu¾É?—Hº²™?æ—VO—î@	íÄoÜû¿³ÂA-œÆJ¿Ý!4ƒqý¿áwÂ^´Á=¿ÞæNþë­ã¿æÑE7Aµ­?•lÖÂïÔ9AGNfsrq3FGL J0803.3-0339TXS 0800-034?ïû`QՆä?6/ì©âv?B~¸©äp<?6/ì©â­?ïûŽ33?b˜\®–J'?AÇïƒ3::?b˜\®–J"?ïïÐ÷èú?lô¹þâùM?`ì/~?lô¹þâùZ?ïñh86ûZ?M°gÖtL ?]/'	L?M°gÖtL˜4FGL J0803.5+2046?ïZV9ht@8ÉDg8~À;9Òïü|¾À<¬@ä@)°-ï#?ÿüS"¾?×7¤¨§ÿ?襢¡€è@	/ËOKE@
³Ë'åö??ïüÕ,ß¿­%ëbd#¿ä'§C¦Gþ¿ïÝu@ô¼Ö¿ïýè-{cN?ïpÿь$AGNbcuGB6 B0800+2046?ïþ£g¤^??5ŒÀ¢>á?%ɅºQ?5ŒÀ¢>È?#ß~?«…£îŸÁ?ŽÕ8·ð?«…£îŸÁ?ìÇñþbBþ?¥°}ÚýðŸ?¹Àpíè?¥°}ÚýðŸ?ï#ëÒîÃN?o(§æ?›'…¢'–B?o(§æ4FGL J0804.0-3629¿ÁC·e
ŠÀ á÷×<'À9ZÙæÃ1À;±¦Ùóü¼@ ¨%o{8?ú±À×ÌP?¹+³b¢3?Í/ö¨=vX@Ýð
¿w@{)(î5Ó¿èÁÿ)%¿Õ¶º¼©éô¿×¯[bQXã¿Ã(™|=h@¿áéñ€‹U´¿â	,«AGNbll3FGL J0804.0-3629NVSS J080405-362919?ï0靐
ß?˜ÎËcuÂ?™âÌMþD?˜ÎËcuÄ?ïë\[°m?{˜Œçž0ë?d㣤O"{?{˜Œçž0æ?êæ÷Ù6§?°VýW;ì?Äd ›«%b?°VýW;ì?ïºó3ØÊ?‰8S"œîo?h¡™"æ¼?‰8S"œîq4FGL J0804.5+0414¿æV>&Ž²$@2.úÆ\À:a(	4À<U°i@íÊt­Ñà@œn`/ë€?¼q{BkŠh?¸LmbÁ?øNI¿f²½@
bK¤™'?ïýêa2Iÿ¿ãŒnØû¯8¿çÎÛ/f¿æú¤¬S¿èX<8d¿ïÿÈl뻥AGNbcu3FGL J0804.4+0418TXS 0802+043?ïû#€³IÝ?L<¤ö¢'?Cqý2؋€?L<¤ö¢~?ïøãC.?jo,=°—?MˆróG™»?jo,=°—
?ïϼûUä?wWֆ™©?x!¸U ?wWֆ™¥?ïÉ÷õË?dÄ\=ÍÅE?{|ø?dÄ\=ÍÅE4FGL J0804.9-0624?Ú÷›3>@*Xä2DëÀ:‡ö'À<'õ»Ÿí@ ˜¢=W#}?üSd"?À©õ‡V ?½=ú·k¼'?þ;ýÝ@³6É?Ïy?Ð*ý$"®¿À
~ß06¿Æ"àå]'W¿Ü>&áì¿Ûm·_þ¿á¶óF´xAGNbcu3FGL J0805.0-06221RXS J080458.3-062432?ï¿Ã)~ÃÚ?ƒ—4]Å\
?€5 O	{?ƒ—4]Å\?ïéE'Ñؔ?y³
 s°?fºn.'l?y³
 sµ?ïˆoYTuc?kÿß×B?ä)ªâ§c?kÿß×??ïÍöäÈ?€¨ÊWÄH›?FA#fýq?€¨ÊWÄHš4FGL J0805.0+6746¿î¢«Lõyl@?䖚
Ø¡À;'çv¯ŠÀ=Ò®Že@¹+x~ÁÒ?ý3o~=Á?ÔJÙã5ÄÞ?ÜדdÌ2s@dZ˜Ó@ºŠ.¾³¿ïÿ–þߙƒ?ïÿ·pD5º¿À@˜ ¯¿ä<UxØY¿ã¬(|öˤ¿ïÿõƒ¥;ŽAGNbcuGB6 J0805+6745?ïü⬽j?@²æ¸??@êš³ï?@²æ¸?ïùt0%jW?ašUÿ"âÞ?J/?jV¦r?ašUÿ"âä?îÈY[öS0?—W¬D7/•?£zj@šÍ
?—W¬D7/—?ï&¹8öžÜ?†Öß F_ž?›(Øá,$R?†Öß F_Ÿ4FGL J0805.1+7744¿ÍUžmXtl@>Z<d4\ÿÀ:ƒ4-.6tÀ<{Wɼ@öFBÚp@]­Z@¾6?¹8¡ èÝ¿³éKó?÷5Ë(‡Þ†@Τ¬È"¿Ð"Ï£@âH¿âFó¤§ê•¿éçåWMÒ¿â©i»…|¬¿ê¦>"z~K¿ïõ¬EmÈAGNbcu3FGL J0807.1+7744WN B0759.6+7754?ïø¶H%-V?Tõ–^—?M&ßkJ©5?Tõ–^—?ïýÌ9¿Ó?H	¾P4Ò?1ž2gÏÆ?H	¾P4Ç?ïÕ³ÒBè8?}£$±h?u&ދä$?}£$±X?ïù6/Žõ¼?:]v`:h?K'AÄ)·?:]v`:'4FGL J0805.2-0110¿í†'»ÀÒ@/"(ÂzÀ9±Ç²±˜"À<,<{±QF@W¨—ä7Í@ÉË«d9?´"D•ÜÑ?Á½…\ @çüMÃØ@ ççÛF?vRdë€Û̿ݲ´Þ¤'¿ç¡&Ö-Ÿ¿æ
ݹ.4¿êö&B4¿ïÿÿ>¹úAGNfsrq3FGL J0805.2-0112PKS B0802-010?ïùщìü?Dš#'Ÿ6Â?H¹ØL
üj?Dš#'Ÿ6À?ïøéSÆpu?cJ'MpÈ?LZ°æ>2_?cJ'MpÑ?ïlÅ.sC?ŠBóCn/?'gZ1œ×±?ŠBóCn6?ïùÎF§?9víh‰†1?KüÆå‰fÓ?9víh‰†-4FGL J0805.4+6147¿àƒŽýĵ@@.}ªOÊCÀ9ºi¨:FMÀ<e(wŽ'@k`ÊÆi@$>úè?µ¶e)O…?Ǟ^ºËm|@
k4*©ø@˜‡C'&¿ÏBi‡¿å¤ÇÛØX¿ë	øÂ!¿é»©Y*=Á¿î_Jé2^!¿ïY/±žsAGNfsrq3FGL J0805.4+6144TXS 0800+618?ïäñP2My?vý-š'õn?k¯Í²‡a?vý-š'õj?ïúÄ 0"Î?g/³¾¢š$?Dï?tȱ?g/³¾¢š"?î'	MÒk?—'óO³?¦ßk"ÙOY?—'óO³?ïüðñmÙ?*ö8 Ëf?88t':
?*ö8 ˇ4FGL J0805.4+7534?é:é£\@>Ëeºnü7À8áhSÀ;ÿ.Y°@Aé~3b?ý&ÈVE†ó?¡'ccý?™_»…iÐ?øéq-iŖ@Lœ«œÑ\¿×öÞN«¿ÕHåL"C¿ßÃcl‹ï¿ÙÏ¾ï"x¿ÛtúÓÆ;¿Þ¬Âû<ÍAGNbll3FGL J0805.4+7534RX J0805.4+7534?ïýŸ.:?*
<Š±Š?3‹‡>+N?*
<Š±§?ïü»ð¬?Lõnhqˆm?: :ŸN(?Lõnhqˆr?ïð°¹6?lZX}Ґ×?^žË"õ`?lZX}Ґ¶?ïë•Ú·ŸŒ?Rã™YHÒ?dj%H`u–?Rã™YHÍ4FGL J0805.8-2331¿í¦v#"+@õĊÞìÀ:ÈlÁÊ:À<GÛZ.I¿@hÝao†¡@*':ƒŽ?Ç刚î®I?²Ë.'?îꀥ+ô?ÿÑɶÂÊ¿ïÏ@À£\?ïùåi{Ĝ¿ä(íßìå¿ãûØSÍ¿à-d‡im¿é¾@_‰ÓAGNbcuNVSS J080604-233333?ïØ?Yªú¶Ü?`yG'áù»?Yªú¶Þ?îÖÓ¥ÉŜ?¼y^
D0Æ?¢'Å£c¦>?¼y^
D0Å?ïÁž\Ÿ÷?}M¡€Ch?0ôÑ°m?}M¡€CU?ï Ë">?‰™5™‡Ja?›ïƍ|˜?‰™5™‡J`4FGL J0805.9+3834?ï÷[ù/èe@>o|¯Ý©À:¸""œÚ—À<ª#}@ëÇ8ä"@ïáÝÖ
?À5a¶©Iæ?˜â¬/t7?ÛIÝC½o@Ð2ÕÀ;o?Òïaz¿±>Y,3s¿æüz9'Í¿×ÙÜÀ4ãâ¿ßÌ´ðã¿ë—p"½'ÆAGNbllNVSS J080551+383538?ïü^Žœ¸A?:®_ÄÑï?=‹=ñ…?:®_ÄÒ
?ïþKñs?B¾›‰D:?+@èÎ6(¾?B¾›‰D5?ïð"ñç³?jž±H?ˆx?^àÖ0š3?jž±H?ˆt?ïõ$u|ºþ?A×e˜ú?U·Š%?A×e˜ä4FGL J0806.1-0458?ïþÞ
{•[@,J•BCÀ;NŒ"¸'¬À<'"ØAu@mö¶@?ùéôÆ)?Ý
¦a©]?ì]d[Ø@§R°Å/@DG?"¥A?Í$‡^X¥Þ¿ïþßÙïÊÿ?ïÚ%`ÙR¿äŠÿ?:Ó¿â &`¼Ù:¿ðAGNbcuCRATES J080608.79-045411.4?ïθíŸì?­¨a'v?xû£‰0	Þ?­¨a'u?ï·3¦Þ¨?¤ÚO…Ç&?'3HUúÑ?¤ÚO…Ç&?î|Åéu€?™ñêÝ5Hž?¨3¡h®‡à?™ñêÝ5H?î]M³¾~? ÔüqÈ)j?ª+$ÄÇ? ÔüqÈ)j4FGL J0806.5+4503?×-‡ùº 6@?«À~à°¯À:µ *­R´À<ŽIöÄ@&üª‹@ð×°´h?ÉÂõ³uã²?ÀT…h_9÷?óNcaÏ(@úŽ±´Ÿ?ïþrâÅB¿é]÷vĂ¿áJ
À2	½¿ìQµ(kY¿ïÿݛQ)¾?ïÑB*òÈAGNfsrqB3 0803+452?ïÿƒ•Ô?#ªäÎR&?ï^en>?#ªäÎR?ïýsz"ú?Q*¿½'a?4d+{X+Ô?Q*¿½'n?ïô5Åô?‡¿Ô'9†˜?‹Âòœƒ?‡¿Ô'9†˜?ï÷÷Cð{·?BE­Ès;?Px'÷?BE­Ès;€4FGL J0806.5+5930?êqûóP´³@@Ig#$È6À:}Æp'9SÀ<«Ù§¦¢—@ ¼²MoŸ@%¥á¦x¥?·gŸïôð¿'¤üñz#?Ú}"ÛF-@£I€C‡?á¶Ì7«h¿ç}€H9Ö¿ã "IÖä¿à%°"±"¿Ç-\"H¿ègõ¢ƒøóAGNbll3FGL J0806.6+5933SBS 0802+596?ïýŒÒޘ¦?*直¢¾?3™i:ÛÖ?*直¢?ïýúù××(?Gh?FG§?0(1AF³0?Gh?FG§?ïûçTn¤?Xg—ó¥
U?Cèb®Ev?Xg—ó¥
R?ïúƒ´Uˆ?4ô€ËŽ½¥?Eñ.©ßáÐ?4ô€ËŽ½­4FGL J0806.9-2151¿ã·ja;e@fð¸»À:ÞØh'À<m¹ô'ô<@dM¢JBC@V§ý	«z?Ê0mƂý?Áw$ºŸR?÷;º‹¨â?ø<N¿ÓÀ?ïì²²$«¿épà'ÒU¿äX§–²^Œ¿Ì\!©s~¿ë~o§WÈ>¿ÑAqºWCAGNbcuTXS 0804-217?ïáBŒ[z?sœü'B?nì½s¤"}?sœü'B?í¯âЅE?¿",'RÞ?²‡pé{ÕÐ?¿",'RÞ?m[ÿ?‰G…@øށ?¤©9@?‰G…@øÞ|?ìÄ@:ª–%?žcEŒ w2?¹Ýþ*«NÚ?žcEŒ w24FGL J0807.0-6102¿ÑKØÙFÝôÀ.¾ó'ªÀ;¤˜ÑÀ<ª^Ô¡­d@¦/ÕÔ¦?ÿÜÀ_×?Σ:Xš¡?×êÈ@ +š@F™&­ó@ŽªÙÝ×a¿ïÿý`éNä?ïÿþó…õ¿Þt—A$¸q¿Ö×=¾ýVW¿ëbÛ, Å¿ïÿöùŠpAGNbcuPMN J0806-6101?ï½r{Zã?'7@"Vp?€¿£a)Fý?'7@"Vp?íó\ÈcÑ?¿sÒ×Þ?°g…¼áƒ?¿sÒ×Þ?ê´à
¹Þ´?¯ÆÅ5?Å,É…-?¯ÆÅ5?ì:Í]iCÌ?¥éà {?¾)•µáš?¥éà {4FGL J0807.1-0541?æö­rD1@,VߋÀ9Š]ÜTÀ;³›ý÷è@v©÷	â,@ÌúÕS"?«ã!€‹ß$?¹"€z䢬@
 sÃF;N@
¶áQê?î¦xÚÝ0È¿ÖE—¤Kú)¿äp5݇…¿àaßyw»¿åþw4ÿì6ã¡¥¯AGNbll3FGL J0807.1-0541PKS 0804-05?ïü6vÒìÆ?4qTJ{/‡?>LIh™Ñ
?4qTJ{/f?ïõÛ>Ëg?hy5ÞÁ;?TI'iÿ0§?hy5ÞÁ;?紐¿Ñ{?… ¼ªÜ—o?†¡??… ¼ªÜ—k?ïîäŽâÖº?I
;'?aq)Ei?I
;‹4FGL J0807.2-7630?ïºKLÊÀ69†3‹HÀ:‰: >BÀ<pâkš'Î@ÁnØå@î€F}?ÃTAöš{—?µªZ±ý>?ò0œë]±Œ@	ÁŠŒ5'ï?°	/(·";?ï lf±¿â-颛uè¿áª}?Æ¿¿ãt¶‹Aè¿éiõ1oä"AGNbcuPMN J0807-7629?ïýˆœû!?3ŸM¥Èx?3¿Ë&ôú?3ŸM¥È>?ïþâXæ?F'ºq½1%?.¾QÚq°&?F'ºq½1A?ïé'ÚûÛ?l5ÏBy£?fØ%$ñ{?l5ÏByÀ?ïêã·Ï?T]YÌ¢^?eH0rc>?T]YÌ¢]ý4FGL J0807.3-1954?éÃë^ã@Ôó…À;e*ýÌÀ<r»H@
²@ØhOõ‹³@V—:*?Ë"-;øS¹?±åޖ£Åí?ëV—¼IÇÊ@Ò¡ÍðŽ?ïï"Ê/d¿ä6A¥¼½‹¿å²>àæ¿ä"8säÔ+¿ÔUÞXæK¿ã!ÂUO"AGNbcuNVSS J080722-195218?ïú…‰"??ûÜ'Þ<?EéÉÙ±Â??ûÜ'Þu?ï÷ÇPf¾:?iæ
e£H?Pq_2ƒŒ?iæ
e£H?ïÝߞ¸¡ú?r²Óî9?q0£¯N?r²Óî9?ïÙ"ݚ-ö?^ÞzNaL?sn'2é?^ÞzNaD4FGL J0807.7-1206?ï!	±žgÛ@%ÂÂ7G"êÀ:~[ãU¥À<;yQ$µÂ@~!IÑ°6@K>WS£ì?ÃæÆÞvB|?ŽZYñ@¨?ÆѾ¿@	è,B©ï¿â®˜™¿YG¿ç²Á-Ý3¿ç[bA=·ñ¿é8'â3n¿åõæ×:¿ïÈc`øh\AGNbcuCRATES J080736.06-120745.9?ïÿ[x²?+SŽXÆy?é–I?+SŽXÆ4?ïûä`U¬z?fÄ<8u¾g?@n~©Nö?fÄ<8u¾h?ïâ²B)ù?nϳ¹âÛ?mM½Öç.?nϳ¹âØ?ïü‡I­ù‰?+
ÕÆ~?;Ų3µù?+
ÕÆÕ4FGL J0808.2-0751¿î¥Wœõ©Ð@*R¾H¥‹?À7‰²gƸ·À;Vd'PÐ@¸éö©?)@å*"8…?•e‰Ç"~¨?µR3S"|¤@ jvSCsó@¸[äWX¿Ä®YڑÜa¿ßÃt
6¿ãk–¼o‡w¿ãž4"䤿æï9©nù³¿íRuÚAGNfsrq3FGL J0808.2-0751PKS 0805-07?ïõô|¿?MÅärÚG?TɁÍ!?MÅärÚb?ï/'"?­(•,ωz?
Û¼V?­(•,ωz?ï¼}Âõ‡—?'"Ú$…‰~?€àBžH?'"Ú$…‰'?ïû=ßò?;¬vBv-~?C샬8?;¬vBv-b4FGL J0808.5+4950?ì}&/v—L@@EA [ÀÀ:
é¿KÚÊÀ<n«ï³x@^'€L–‡@¨1­!5Û?¼µ#7èz?¾Ô»-½þS?ù‰žsóî@©A,p ?á?ž{«¿æ¶<½u–Û¿éfæÀ¿ïL´ÔQP¿ïüð¡=Qð?ïûûùáAGNfsrq3FGL J0807.9+4946OJ 508?ïúã­µ—À?XM_IcCE?DqI) ü±?XM_IcC;?ïrâ®Êi?©Ï¢ŸòQ?'£ª&²Ýò?©Ï¢ŸòR?ïǨC 5î?{ŠN"n¹:?|+Þoåì?{ŠN"n¹;?ïYÀwEë?‰ÎT6 º?"ÇüqB¾?‰ÎT6 »4FGL J0809.3+4053¿êº˜5×Ä@?""åÕ²OÀ:Zi¡"I¦À<yèÿ2z§@ög¢{•x@ü6ڇ s?Á¨wB¯Ã?ºzÈH-Á.?÷ oz@
6H°HÕ?ìø´¢¨ñ¿æ6¿áa¿èׄKS»i¿ásï@j(h¿ïÿð°×£À¿êëÒ¶ñ™5AGNfsrq3FGL J0809.5+4045S4 0805+41?ïü'évÙ?@ÞÖÞ:-??ûp´I0P?@ÞÖÞ:)?ïü¦`5,?Mnƒý½K¯?:ÏüþV¨Í?Mnƒý½K­?ïèåV|ʒ?fŒ
6­?g©ƒ5mÈ?fŒ
6­Ž?ïêE¯ÿ*)?SB¶?eºPÕ×Í?SB¶
4FGL J0809.5+5341?ÔQõNu@@vQ ÄeÀ9OM½øôsÀ<w^o@ÿ½ð÷4@QâZӋ?®2ó'Þ?¼ç—~aYâ@¶î·`-@
+m—C¿á+}âƒî7¿Öļþ"°.¿ä­'Lž>¿â±4Ur"\¿è"âÀ*'¿ïÿûbâMhAGNfsrq3FGL J0809.5+534287GB 080551.6+535010?ïü¾î®ê
?4™ù3cª?:Šˆ¯¬!?4™ù3c ?ïúòe‡~?[ævI »í?D5ÊiâÉ?[ævI »é?ïg+õ²1? ¶. pŒ?"I¾™Ì? ¶. p‹?ïÿ#Ìíò¸?
œÄ1 g?†bA¨ñz?
œÄ1¡¤4FGL J0809.6+3455¿ÛhC"ì@>[=ÀTïFÀ:—öÀ¼RÀ<…¬bäÒ@ ìKœ%?ü­,SE!r?¹½0EÃ?xHÝ%Ï6?±o¤'½@çèF¥Ö¿?ï…[ôó]?Òà™ËW'¿ÝC­iZ6­¿Ô
ÿx›¿åOoù?·î÷€:ß
AGNbll3FGL J0809.6+3456B2 0806+35?ïý_—i9»?3èwáé?5D¶23#?3èwáé	?ïý£
­wˆ?H]'¼³A?2窔CËÀ?H]'¼³8?ïô¯}‹•_?\qôˆ?V¡èÕC"?\qôˆü?ïêÂ"&?R³=ÿNJ?e=üílÚ#?R³=ÿN:4FGL J0809.8+5218¿îó7ç	‹@@uÂôÀ7ßF€"À;WFG.@ѹ©™è?üúÜà@G?™úAú÷,? ¯·=C'a@Æy{ìài@/®'MoÊ¿ÈKÇ©¢PL¿Û ÿ-C¿ÝùVÆ'!¿Ø`Z³ª¼Ø¿à҈˜ÀUÆ¿ØÿŠÄê€<AGNBLL3FGL J0809.8+52181ES 0806+524?ïþ¥vÃél?âðCæÏÑ?%¨"ÁiCK?âðCæÏ^?ïüÁ™hÅí?SɱŒ£«¿?9ó4¹Ð"?SɱŒ£«¿?ïàqì
må?rË°–`â?oŽõ'—?rË°–`Þ?ïÿ¹Ryqã>öÌPxò#5?«a£‡â>öÌPxò"¸4FGL J0810.9-4926?妜s‡oÀ!8÷‡‹zÀ:·SŽÕÀ;ó¥è\uL@'ªk¤@K€œr'î?Ìw›Žy?¯ðRAâ?äSõ`æè?ყòͽc¿çµfI
5
¿ã݄ªõ°¿é…Áàà€¿Ý8Îø ¿åÇM1:Ç¿ïØ¢žP³AGNbcuPKS 0809-492?ï†ÃOÐL?¼×µŒê!?ŽO,þ­8?¼×µŒê!?íôC9þ"?¾à2Wµ>M?°]æ0gá?¾à2Wµ>M?ï$˜ç?'îiꕞ?›LÿœÃ?'îiꕛ?æÅEbù;m?µ&¬©û?Òuu:
‰'?µ&¬©û4FGL J0811.0-7529?çoÿמ`CÀ5r=_ÜßjÀ8~é°2bSÀ;ŽÅ=jÅ@ÎȦ!'L?üûõ)hÄ?£pî!'ºQ?³@ÒÙb@{Sþ"Õ½@	.¡Kϖ?ï`ø0'æ¿ÔžÜÏyOw¿Þ_
agy¿Ûé¯Çˆp¿áD…Àô§\¿àW}à€ˆÑAGNbll3FGL J0811.2-7529PMN J0810-7530?ïæˆÀ®Ó?kî.bpx?iîw?Q,I?kî.bpx?îæÚÆ	d?ÀMY¾az?®'SŸi²?ÀMY¾az?ïR0[?—ç*èË%?•¾yôœð?—ç*èË&?ìp\ù™N? ‰G8B³à?¼å35? ‰G8B³à4FGL J0811.4+0146?æL
ôÉv@2ìAÝ"À8ð&n(ÓÀ;nÇtž8@G4 ñ|¯@üÉð?˜ÿjÙ½¡?±ž
áXä·@]û¹I@³¥ÂqÕ¿ºž'úb¿ÝxÞ8/¿á¦.ÓR"¿à· ÈÍcÌ¿æHùµ¼æ¿âD`ý›Ì¥AGNbll3FGL J0811.3+0146OJ 014?ïüp,éò??5juS4¢f?<~˜°mÿ;?5juS4¢p?ïëtڒ›?~OŠ?d‹á%mdø?~OŠ?ïÏe¾#€?€--a(Ù³?xM î?À?€--a(Ù¶?ïýg›ÛD?$š8#ðù=?4Ã!'ÝÞ?$š8#ðù4FGL J0811.9+7847¿ï顦€"Õ@>t‰ãC0×À;Z¨®àR¼À<£¿Ü#å@úËܑ¼?÷Ud;ü?á"r&Ž	?æJ 'l"@Ž{Xeó@gî¸/ý?ídIáJˆ9¿ëÇ€\±²¿Áã˜ËéM¿æ¤á@¢1™¿ïü#åGî¿Óè5=ÏnhAGNbcuNVSS J081307+784308?ï—{A×ñò?Œ¾?³ú?Š!/Šƒs?Œ¾?³ù?ïíä]µ	I?",'oí‡?b¢Jöµ?",'oíˆ?í–nQ~OF? ³ÛÃ?³Lt
…Î? ³ÛÂ?ï$MÛ덹?/],œ?›vD'ŽHÜ?/],œ4FGL J0812.0+0237?ïçk³ÝÐ@3ÚãæÄÆÀ9ðËЮÚÀ</°r#3@ Îý~›f?þÝΗ¨'Ò?¶Éš'ª·¿™UpŸÐ?s?㝺|h0?õ ôg˿1f™'?î
üwµCC¿âÆAp㘿Ù*»*
Ä¿àcJB~Q¿Éy—›'˜AGNbll3FGL J0812.0+0237PMN J0811+0237?ïñ`¾?aÔ8m¤‡?]?ƃÕݞ?aÔ8m¤‡?îa†>ПY?½õ—{Òxi?©çœö
v?½õ—{Òxi?ï¸Gæwàl?~×_K=+Ù?îbå??~×_K=+Ø?ìN]mªž?«aÆV%­Z?½'¯Ã?«aÆV%­[4FGL J0812.3+1143¿æ^¶!{±Î@76OD
ñÌÀ;«°óRsÀ<‹Q$µÁî@ͳLóùŒ@ÞÖ4T›c?ÎAƞàUk?ëqÈÅ+C?ñlÐÈÚÏÅ@±´›Ó†?Öñe]|ÝÌ¿ÔÿcÍÚ¿¿çût_ÎFÊ¿ä#@v蕿ïÿÉ
ûkF¿ïÿ–þߙƒAGNbllGB6 J0812+1141?ïÔÈ{i?y«TÔ¹ Ú?u›Â}Kpb?y«TÔ¹ Ú?ïälö1L?…–øDr?k"	íδƒ?…–øDr?ï[2k?'דÓüÁÃ?ž™¯ÍòØ?'דÓüÁÃ?ïƒÜÑò?Â?vù¸T¹¾]?˃p?vù¸T¹¾\4FGL J0812.5+0711¿à
½S»g³@5LP&‰ÅÀ:Ë7š¡–À<qe/.Á´@wP3:@
¸A$?½µ˜'ԅ¿‹R"Sba?ÅÀ›{œª@ˆQë…¸?ÛÏa×`z¿ë¢ÎLT¿æD‹ë[-M¿àâ4½÷ÇÍ¿åŽ)Þöšü¿ïÿ¾úAGNbcuMG1 J081238+0712?ïýo|Ì;?8M‰~`ž?7"ž*«?8M‰~`ª?ïþUž?IÌY
-Qä?.ª®?F(N?IÌY
-QÚ?ïìT!U®<?fë£WÄ7§?c«ÞªQÂr?fë£WÄ7¨?ïûoÛe?3²l¥ìéð?CŸ¶@'kå?3²l¥ìê 4FGL J0812.6+2821?æ,IqeÏ@=9Ñ쒛À:ö ‹Â[À<¨7Üæ @ƒ	ðï–Ñ@&÷ãÑÌ?¾r`ßW®¿¨õF'_/)?îA|7@èÈ€ÿ?ïåÔ`Û?ï½ö¥ä*·¿é˜+ˆ¿ãz?–îÄn¿ÊÓ_ãëL¿ÔÏÞЏ²AGNbcuRX J0812.5+2820?ïüxXé+?:Ä¢GpFý?<=?8¶ª?:Ä¢GpFÊ?ïþ+[žÁÈ?Cû$'í* ?-JFã‹ë?Cû$'í*?ï×ÅU@h?y ×#¾<?tU_Ëõ ?y ×#¾3?ïõxŠÞؙ?G‰"ûhÑ?UêBNÐ[?G‰"ûhÄ4FGL J0812.8+6507?ïŽÍž:'²@@y§~^ª°À:žÌZ·»À<š€ÑK·Ž@ 'Íút@wßÖjÛ?¿kÂ_¥Eä?ŽŸj~y?ÐîOá?@>!œÀ–?î)Ý´{/¿èÜÏ^w"œ¿à'ä¾Ûó[¿ä"¥¡º¥X¿áԦ˱D¿Ë7Qzñã³AGNbll3FGL J0813.3+6509GB6 J0812+6508?ïó'NÀ4í?T•¿_|?Xûb–#ß?T•¿_|'?ïúóÏüà?Z_n%2"?D0À€ƒ
?Z_n%2•?ïé-a6qi?kÅ®Êݤ;?fҞɎ–Q?kÅ®Êݤ7?精ÀQ¦ê?q~^¼ªFe?…؏ë–E—?q~^¼ªFa4FGL J0812.9+5555?Å7‰ú@@»3ÞLQÀ:þ'œ&;ÔÀ<¼MÑD*Ò@ ž
Lµ@CHÚde?ÃMИ^[*?"V±^ÿŒ4?Ђp½Ø=C@Àõܼ?ê80Èõ§·¿ç_&DÉ¿æ€(^ÃÚ¶¿×ì"é0°¢¿âBÞ¡áf¸¿ïÿ¦¶tFAGNbll3FGL J0812.9+5555NVSS J081251+555422?ïþ@K¤?'dÛfdK?+ûG%¿Ö4?'dÛfcâ?ïþHWž°?E`˜yÄ`?+z†÷3ï?E`˜yÄq?ïøCoô£o?T¨É!«?Nò@-rD"?T¨É!«?ïõÎ/¢Õ·?=‡pkÇÉ?Tc ºT'T?=‡pkÇÌ4FGL J0813.7-0356?ïò¬?Êo@0Jò"z–À:Ê/•ïÀîÀ<p¼Åd@!T(Ì'?ú{¬\ë?Èôî~ù/V?Ç`1Ùkì@J¡äÁ¶@;DI[Ë?ÔC¹"4$Ë¿ålüþóg¿µ…(ÞÆtn?·)£dm­¿ßüEá5ºw¿ç$8YáAGNbcu3FGL J0813.5-0356NVSS J081338-035716?ïõ†Hϕý?T'L ¸ék?Tón`ÔT?T'L ¸én?ïíˆ@/*?wœþ›}Uû?bùw¿ÐÔn?wœþ›}Uù?c¦`aÄ?~Jõ'²]E?€Ÿgç	?~Jõ'²]G?ïf'ã0Ùû?|/µ:p¨Õ?"/£™äÀ}?|/µ:p¨×4FGL J0814.2-1013?êË~Zæt@*m¾]ž@ÈÀ979_JÀ;ødÏ@ûÃ	€@•{âÏm'?¯©¨|Ø»?©^v¿
R¥?ú±ÅÅqŽ¹@	½Õ{G"?ïÿÿÊPË¿Ú$'óÕz¿áÒ¢dCvw¿á$Øâ"Äö¿äŽî_ċ¶¿å›«–òAGNbll3FGL J0814.1-1012NVSS J081411-101208?ïý6yùs?4¹±¦¥ü?6O404eÆ?4¹±¦¦?ïí˜yµã7?}6jåµæt?bg†JÉ1?}6jåµæu?ïß:«±†­?tl€Èe?pbª'<ª?tl€Èe	?ïšRBÌ\é?tçp€Ý&ù?‰koLèÅñ?tçp€Ý&û4FGL J0814.4+6926?ÌBUç±aÒ@@C3‡	WÀ<0€sWæqÀ=+ˆlJ«ö@"òÌ!V;÷?ú	‡¶Õë?Öxë8Ȟj?É¡ú{±§,?öD?Àà0?ÿƒµl3¿ïýv¸ÄL¿íEIJ̬ì?ïþä­³,?Ë¢Ú`S¿ââÝ°IßG¿ÄC/ÀAGNbcu1RXS J081407.6+692549?ïüµ¢¼"_?7Ñ8ë z?:Rêe?7Ñ8ë t?ïû-`b߬?cÑ`U'?CJ~tSÛ?cÑ`U"?ïÁ2/_?~À'bÿï?æèpÏò?~À'bÿ÷?ïÙËuߌ?fÔ­¯C£>?s~E:{?fÔ­¯C£?4FGL J0814.4+2941¿á?"gÙÀ@=üGõbÀ:õl‰–WÀ<'@Þí`Á@ ³»Öƒó?þí@ÅÂíP?ÈcF¡Oš?²b["Ñ2ã?êÛª ¨»?÷*&ˆó?ïþР@ý¡¿éËßR,¿Ú¾/Gì(¿Üè'¯qr¿à姏%¢¿Ø¦á€¸øAGNbll3FGL J0814.5+2943RX J0814.4+2941?ïþª*¢»?$è#="?%]UÞ4N·?$è#>?ï×ïj›b?‡Íq,RÉ¡?tJÀ2O?‡Íq,Rɟ?ïì$Hƒ?kñHy™å?cÛ·ýí}?kñHy™å?î*q¿?"5é节?­^/¿èä?"5é节	4FGL J0814.5-2642?áÖÙoÙ°@ªžåXµÀ:Ç!—)|ÑÀ<=ŠV/·~@tÿKû<@a$z2Ì?Ï«b"Y–t?Ó½Éd7
@ SŸºE@\—rÍÒÜ?ïœø^Kò?ÕÖ\îm†¿Ü±,]Vl¿æ«Ý¾â~e¿æ'ÃÉf¿ïÿÚ`‰,ºAGNbcuAT20G J081427-264422?ï½63¿@?"¡rà®?€¾2s0J?"¡rà®?¶–hž?£¥ãç9N?ˆ\RZeؾ?£¥ãç9N?í¾D@ĺÔ?¡Qv…\Jf?²
ÝùÚ)Z?¡Qv…\Jf?î¿bRSdÕ?‰LàŸ
?¤	ÚÚɲ?‰LàŸ
4FGL J0814.6+6430?äiÆ*¾[@@šb=ú	À8©ƒEW"À<µê28a@>Èáè@Á£n.±Ä?žíC\B˜x? XÑÓFäk?þvk+Èç@/¢ÈÂQ¿ßLVð§h¿ÜgÇúÕô"¿äuð²…"ê¿ãsÉü7ô¿ä¡^E°Ž¿æ%ÜÓ«
_AGNbll3FGL J0814.7+6428GB6 J0814+6431?ïü¯ê%­?6N)v1Qn?:€®Óz˜ì?6N)v1QS?ïûfÿeš?Y
ü§Ó
?Bdi¼?Y
ü§Ó
?ï̓`û¼?--å|?y}>O'!Ü?--å?ïø¥Ã‡KÖ?B;'9YÃm?MhñâЦp?B;'9YÃv4FGL J0815.6+3641¿ȩ̂æûï·@?ì"F{åTÀ;ÿ!³®ïÀ<˜­4
@-£ôfnÊ@[¡/?Ê_d©ø·a?·oÇäÌÃ?ï2 Ñœ?f?îÅ.S-,<¿áBÓNÇ
p¿Ë@%	#ë¿ê¸¬"Wé¿ÜÕ¬˜¥¿æv¯Æ+É¿ïþϞŽKAGNfsrqOJ 320?ïފè†z×?|
­DHŽZ?pº‹¼Â"0?|
­DHŽV?íÚì	â#÷?¼¾Jø{?±(Ÿ°îàN?¼¾Jø{?ïN-?kôÌ?'R= Ô¶á?–:Xf"?'R= Ô¶â?êaPòÆ?¯;{Ɯ?Æz¼7ÿ é?¯;{Ɯ4FGL J0815.9+2951¿ã½S4lšÝ@>VΚ,fÀ:ûàÊ°'ÚÀ<q±6nQ@E´%¶óÈ@zvSCsó?Úz}ib?×r2aüõ4?ÿ‹µÆ 
b@Ùèú)ý*?ïÿ~‹¡3¿àLÞÕãÍ¿ÔôŸd3Ü&¿è¤N"áÉ´¿ïþ8µS3"¿ïûÀj¾º»AGNbcu2MASX J08153642+2950218?ïæ¶:Ÿ;à?rU«ˆ±ê?iIÅ`Ä ?rU«ˆ±é?ïÃnwœ?"/A8ïë~?~HöD1ôh?"/A8ïë~?ìé×ÿõˆ"?¡´|'—?¸±@S»u?¡´|'—?ì쨪ç9ä?›Ü'ƒõ?¸šº¨Æ0Ý?›Ü'ƒö4FGL J0816.1+4909?íñ[½W@@Ü!BoçÀ:·HIÑÛÀ<«¿2°Vu@=>ô‡|@-Ðãe–?À×h‡'üô?°åä Óö?ðbE¥%¾Ö@ùì¿0þ?ïÔ\
G`¿×ËïW;P8¿ãGø½Ÿ¤¿Þƒ.ž#¿ÞNy	×W¿é#7r]®AGNbllNVSS J081609+491005?ïòÅzè?SÝ°Gö?ZuÒ/ßÆ?SÝ°Gú?ïù8Šæ"?aD¬Úƒ?KÔgxA?aD¬Ú‡?ïêÚAè?m6z@	4Ï?e%â¾ê¹?m6z@	4¶?ïeûèP
g?xžf$E?"@'õþ³.?xžf$E4FGL J0816.3+5739¿íÔÏGõÄÖ@@ó¬Äï‰À9'—¾WÀ<1áÜ(Šc@Tåÿù @CrSÍÝ?¥ LâÂé…?¬Ò½–gÐ@¶ÖU⊤@¸õh¢UÖ¿ã~É3»o¿ØG"ÂLÁ¿â±ðrÄB»¿Ý"²œõē¿å¡…¡?*b¿à<	›Š4¢AGNbll3FGL J0816.7+5739SBS 0812+578?ïûñÎïB7?7~+­!<é?@8ÄB÷"»?7~+­!<Ñ?ï÷öãø±?eŸº®á
'?P8òi?eŸº®á
?ïéB@ç¡?gö"X:eÊ?f½¿€_?gö"X:eÄ?ïÁvSÕTÝ?mC÷ x"8?DÖU'?mC÷ x"24FGL J0816.4-1311¿åÂ¥ë÷ü@(> ÿT–À8ŸªúêíÀ;Ÿž¾œˆa@èð!Å?ü®»iÍùó?¥xÜI'Í?©Ñyž–Gn@u¦uJ/@ÆÑÜV,²?ï÷$ŸF¬¸¿Ýƒž›3»¿àŽ¡¹"ËÝ¿Ó禆轿àce•†¢¿Ùf=̔CAGNbll3FGL J0816.4-1311PMN J0816-1311?ïþÑcv*¯?³æ}¢¹?"éȝU%ð?³æ}¢¹?ïõ]–"¾?q
®/¥_?UDÓÎք›?q
®/¥]?ïÙ!A¸Ò?wÈ(ÕÓ?s|o_#–¬?wÈ(ÕÓ?ïöÛq×?@çnçŸA?RIzÞS?@çnçŸ54FGL J0816.4-0007¿ïôP7!nC@2Å3	AÈ!À;+÷­K'FÀ<y³J@å´Ð+Ò?ãÚPx¾W¿?ß4þúÇ[õ?ïqèEÏ?úΘ´—Ká@帧ü³Å?ïþÂ^§U¿îPªJè¿Áb]åc¿ËÑexTÐg¿ïÿJ=eç¿ïÿÿ>¹úAGNbcuNVSS J081626-000559?ïûM=ŸG?Q`´âk1y?BË	'â~?Q`´âk1{?ïô2ø€?yµc*þÕ?WϛÒ?yµc*þÖ?î52à;"?œâØw?¬¬ÖñüFµ?œâØv?ïÇýÖûu‡?wùev‡ð¸?|'E=6?wùev‡ð·4FGL J0816.7-2420?è(Ó±uæP@'ܱF^‰À9މÁµA–À;ÒWF7ò¶@1f]×÷x@Š(ãN'?»a'þ0-V?Æjsç-v0@	¯å†6a@ۉ–AJx?Š‹h(ˆ_`¿áU±wÜ°p¿ç8Ò¿€#¿äi+<Ĭm¿ì~Ø;•Ø¿áâiʀAAGNbcu3FGL J0816.7-2421PMN J0816-2421?ïCÈZ¦?˜™æÌî\ì?œ÷†ô«=ª?˜™æÌî\ì?ïõéXzŸ?pYa¼Öüå?T-O
ÁÑÂ?pYa¼Öüè?ìД
]ïÛ?¦£ô"ø2?¹{_­4?¦£ô"ø1?ïÔåÏY_?b¦ø¾ßz?uy˜SO¶?b¦ø¾ßv4FGL J0816.9+2050?ËSÍvlÑ@;»ä›«—À:•"¿e=À<f:N°g;@·ëm÷ªF?û<¹t*tH?Â2¡èȀã?È×(ñ:ë@Öoþ•œµ@ãbý%Z-¿â'úÒD?ïû(Êúd¶?'½¨d-ٿӆ÷ µí¿ãð6(°ù2¿ãÂýuâlAGNbll3FGL J0816.5+2049SDSS J081649.78+205106.4?ï5z‹Ó@?—v–K2Ìæ?™_°®…˜?—v–K2Ìç?ïƤ0¬·?›. µV
´?|­çü©¤Ñ?›. µV
´?î9+ý[f? Ìöõi¸†?¬m@*OIž? Ìöõi¸†?í°Âê†$ð?–dªpF$<?²yè«Î؂?–dªpF$=4FGL J0817.1+1955¿æoj•ey@;rÍáŸÂ©À;JžWn{ßÀ<£ô¬å¦¸@!±=®6^·?û'êÊä•@?ÏtOȸ–?·ùÓ;PŽ?ꖎý‰X.@Z_Çæ´¿ïù·FRʨ?ïÿü9¡â=¿Òfý:'￶'êΕyÏ¿é2IÉw­·?ÉGŽAAGNbcuCRATES J081705+195836?ïýTÌŽ?3݉ñ®Q?5YŸÇ{"A?3݉ñ®t?ïü'Pÿ â?S'NGD?>Åxøõ²?S'NGD?ïši‹ià,?…Rµ`bê?‰e%‡õ?…Rµ`bç?ïÇDw_ÿË?q!¿½YŽ?|]ÄP÷?q!¿½Y4FGL J0817.8+3243?â'ë 4#@?{y¦µÀ:¯*‰@†À<pê?«ç@ a1R]oó?ý@"Êý¿´?Ï:N°g;x?Èü†c[ïë?ûòˆcp'?ûnºÖ*C ?ïgI}!"¿à–ØŸ8¿Ëñ†ÕòV¿Øx$>x¶ ¿à'¨9p¿éØæZgAGNbll2FGL J0817.9+3238RX J0817.9+3243?ïå÷Bho­?eêñjò°?j½—Rg?eêñjò®?ï¨ñµŠ[?•Ä5B\?…Ã'¿Ýi\?•Ä5B\?ïl)rÍ…?êZj?'zѦ]¯y?êZjƒ?ìPïöWø?ž6ØÅ{?½x€MGøB?ž6ØÅ{4FGL J0817.8-0934?é_ÞEiÔ+@,¥hÍJ¡À9÷І•±À;¾Ñ"Âr@«è¦
?þB>ƒÉM¼?°	ü-7›£?Àñœdûi@/ô÷í@	[wÿ@"?Í 18\<í¿Ø¢°=w/¿Ø8}%Ō¿â<a_–h¿ä|PKߧ¿æ"z~K_zAGNbll3FGL J0817.8-0935TXS 0815-094?ÔÜl'?†yÛ/V>?‡ÚŠÈäۜ?†yÛ/V=?îUåŽå_?¹Þ	Œð?ª¡¯7ª	?¹Þ	Œð?î|0ÅÐL?œø¿½‡Þ?¨<ó¢û7û?œø¿½‡à?ì/Z?œq‡[À˜?¾‡/÷ƒ?œq‡[À˜4FGL J0818.2+4222¿å/[²C@@²`˜À7µx!yÍKÀ;lðå°Éa@'ä6>U?ÿïCZD?–µc›þ?µ@j~N¬@ ­¸d"@V{Šæ¿ÄB1¨Ä"Õ¿Ú$¡4˜Ž¿â[Ã?…Q
¿áçø¢=­¿åŠK1Þt¿é3
ƒç€­AGNbll3FGL J0818.2+4223S4 0814+42?ïîâ
?ÏÁ?]K÷ƒ‡µ?aõÀ0@d?]K÷ƒ‡±?ïËN©eó?á3!}ý¶?zX«Mz¼?á3!}ý¶?海Üÿ)¡?ˆ^•Ôb?…žˆÀ5—«?ˆ^•Ô`?î¼jFŽx?'w§ÃØ?¤9_ë—t?'w§ÃØ4FGL J0818.4+2816?î­1óI7Ž@>là¨KäÀ:ªp-…DÀ<‡ËCòž@šÞ‡	t?ÿø€¯½È?Æ3©Ðži?Áío"3,?ûÂùå3Ì@5½'"Aç?ïÿqÐ&ôa¿ÔÆÆ"Ž ¿Ç¦F{9‡5¿ç骾…m¿Ó÷V
RÎڿ㟟m1AGNbllGB6 J0818+2813?ïþ‡·oM7?%Æì?©?C?'"‰,¢–?%Æì?©?k?ïý¨ö–Ú?HŽs"
ŠÂ?2¸KI/åÒ?HŽs"
Š­?ï½äŠŽ?ÀV?€†Ý\|ÜÉ?ÀV?ïޖ1ô2.?Z·.ßæõa?p´çæèù?Z·.ßæõb4FGL J0818.7+3153¿Ø7ÝLߗ@?vq%Ý	[À;]r{ÛCÀ<´°X"@½ˆÍC•+@‹t"Ì?Ðԍ çìŽ?´˜û(·¯?悬î
46@
½©y
­Ù?î9Xç!â©¿ëL´,j?ڒ1%;ù«¿âg‹_D36¿ã÷÷ˆb9±¿ïÿæ¦SfAGNbllB2 0815+32?ïÿwbO=?IJˆÚªÃ?¼XY?IJˆÚª ?ïþŒOîéâ?B""~¢Ê¡?';aì
?B""~¢Ê?ïïý;ä7?k3/ð?`Äôș?k3/ð?ïû&gµ?2³3Ÿ«†?Cfa+«•ª?2³3Ÿ«‰4FGL J0818.8+3229?ҕœ|°µ"@?žbÜn*€À;.'4ùÀ<b¸®1×@Áœ/ñ	@!"U…?×Â$g¾U;?ÁώÞ§«?ð4Ä}ròf@«Ð9h×Z?ïÀ«÷j/I¿ãÓîÿý{Á¿éq®~-,‰¿à°!/ûpN¿ç&[L
¿ïíp±C‹AGNfsrqRX J0818.9+3227?ïû
AA=k?PÚz¬së?CÖúû
V?PÚz¬së?ïýHM?Jünój¡?5¿Ï§}Ž1?Jünój¶?ïÒªÀ`bÂ?€uîˆ5úZ?vªŸÏΞÌ?€uîˆ5úY?ïÌE|Uæ?dl °W\]?yÝAÕôþ?dl °W\Z4FGL J0819.0+2746?î|LähO@>j;šàÁvÀ:v[ËرÀ<y¿¼CÎ@‡ފºY?ÿ'è_ÐJ0?ÉIøÜö¼?Ä`EKc¬?ý&ðš1o?þ¿Ý/ñ?ïùï2b¿ä´Ø"óÙ¿ãã9Ü>Z¿×Nø 7­ì¿èLˊ­n¿ïÿÛLÂPrAGNbll3FGL J0818.8+27515C 07.119?ïßb'?uÖ´º&aŽ?pN¶óóôÆ?uÖ´º&a?îü*"g L?±R|‰´ú…? =W¹…û,?±R|‰´ú…?ïZèŸ"?ŽáX,»O†?"¢ü,¼•?ŽáX,»Oy?ëÆ_7òÝF?£È£8ÎK?Àæƒ 4Šç?£È£8ÎK4FGL J0819.4-0756¿Ô''¸ZD@.úò¥µ1À:¸—/\À<igÏòñû@!™9ÍV5?ý?cr–'?ÄG?D8"?ûžû?Íi²KAG?í°T¸'×¥?ï³~è=k›¿é°iS¿å XóÖ&¿Óˆ!Äuæ¿ÖM
ú¿yR¿Ý¹žrAGNbll2FGL J0819.6-0803RX J0819.2-0756?ïü½¾w?<YÁ"4?:GTJ8?<YÁ"(?ïDÍ!ìò'?«¸ÁÔFäé?—f[Âa­²?«¸ÁÔFäê?ïé]•Ä'–?p=-"85Í?f¢j;mi(?p=-"85Ò?îã̒´?"ُÏ\çr?®ž1Ã6Ô´?"ُÏ\çr4FGL J0819.4+4035¿ÐºÜ?_Đ@@­UÅ.rÚÀ;ZÄ"ðÀ<ÀëóÁ{@ xE×Ћô?þ©Úª!¨?ÌÕ2÷Ï
?±:‰hÉíõ?áDø®ÖÃ@<pŸû2'¿ízÝð,¿âBMb3{Ø¿Þl~Q¿Í¹±<"›¿æ²"L*zþ¿Ý1a¥1'AGNbllGB6 J0819+4037?ïþ¯Ÿ‡3L?†Âz6?%ŒËJ…?†Âzj?ïý‡"Pv>?M÷E%½?3Ãe|N?M÷E%½?ïõ•lè†d?cÞ«4g?TÕ&.ó:^?cÞ«4g?ïó û}5J?G	²Ä–5?Y¾	•iF?G	²Ä–54FGL J0820.1-2801¿íöKê7*>@ä—t%kÊÀ;nE£x?­À<ŽOËð-û@#'Òëò_?öø¼ßï¿@?Ñúj>ã¸?ɒOù<—`?÷—%¶rî4@á)`Ìt¿ïÿþÐñ?ïþ!xöŒ¿ïÿã_¶Hý?ïÿð`OËð¿ä2M?Mó©?ÁcÄÄÂAGNbcu1RXS J082021.9-280206?ïù%òç#T?JÜ­49£?Kh4cr±q?JÜ­49Å?ï3]Ýëõ?»èÕ?ØËX?™"DB]&?»èÕ?ØËY?ïTŠ'¾ó0?Ç"áïz?•n¯¨!š?Ç"áït?ïÅý˜ª,a?~$">º-?}3ªéϯ?~$">º-4FGL J0820.3+3639¿îeìz´nL@@l% Jù#À:,Ú"ö¥
À<uo·HJ@Š%»üE
@"€Þô?¶èô˙q?¤Òhÿ./$?îRœàKß@½½"J¥@¿Ïœ¤ç€'¿áÁ÷Tð¿åùéÀÎfÖ¿áyPFGã¿ånbHÊt-¿ç!ñ¢DõAGNbll3FGL J0820.4+3640MG2 J082018+3640?ïñ¬sÕƒ?VO‰Zé?\§UÈûX?VO‰Zï?ïüÍ\ýR?QÄq[0ð?9•xiU?QÄq[0í?ïê	üT	C?m®ùîy…s?eö«ö½F?m®ùîy…x?ï¼7´¯N?j=¡Ð+^?€òøÔ,Ò?j=¡Ð+^4FGL J0820.9+2353?"Ðñ1Ð@=ŸÑx-8GÀ:ÎQ1JüÀ<yôÆ)@¬K&ÄåÎ@l#ú±¦?¼¨ñPdÇU¿²†æ¹‡÷?ô?I)>¾@5."hƒ¿åñ¡mx~¿èOÄÎщ˿äÐà,Ðî¿ã ÷&<ª«¿àWg€桿Λq ?[AGNbllGB6 J0820+2353?ïðbð…(ž?\@¨£å?_:õ®ÃÒ?\@¨£æ?ïý¹Q8?I¯ï¹%Ùá?25wV?Îx?I¯ï¹%Ùá?ïågS˜?tZ»€Ü"?j˜¬ãgpµ?tZ»€Üy?ïç‡VKõ€?TãBóáñ?hx©´
~É?TãBóáè4FGL J0820.9-1258¿íGàR÷Sá@*X©XS~,À:z:iˆYÖÀ<^ߘk¥@֊þÌ#Z@ɀ¤Ö
¾?¿3~݀¤? ÅoôZ?âObcøM?üû@}ž'?ï×.Ož£Å¿àA0íÕ·¿ä%"S·79¿ã%aE•6¿ÝrqÂ:!º¿ïûOyxAGNbll3FGL J0820.9-1258PKS 0818-128?ïÚ¶bŠù?p&¾wƒk?r¤Îºƒu?p&¾wƒk?ïÊûQ©æ?"úz§ø
?z'~×+
z?"úz§ø?ï´ÀûµÜ?€¼ÊÑͱ?'ÏÁ‰#?€¼ÊÑÍ­?î÷@%¢0?‰Ȗ9"µ? ‹ý¥ß?‰Ȗ9"µ4FGL J0821.1+1007?ï_Rýøç@8~»˜Çâ'À:ʺ?+ŽúÀ<‡Q\&M@4êÕeM@…ôäC?ÀxD_U{¿£*RŽîù?â†i`Á¶Ä@
SÉÇߨ¿Þíӄø¿åSŠS«y¿èœ!3Vo¿ß[º9¿ä¢aôçž	¿Ú|=&|AGNbcuSDSS J082054.81+100609.4?ïþ8óÜð'?&¡,cȒ?,pÂ0÷äA?&¡,cÉJ?ïþ¶ µCL?D°Øñ]Ã?$ô«Ë+Ä?D°Øñ]Â?ïñê3$mƒ?`ö]ß#ì?\+™·$úF?`ö]ß#Ý?ïý¸v%ÌÇ?!0ÉäÊWü?2<Nљ¼û?!0ÉäÊWÀ4FGL J0822.4-2630¿Î:¢™éAž@ãS÷ÎÙÀ;
1'rƒ«À<_")P@0<yûš@uØå	µ?Êúv=Éå?µù…½n¶?îÈ.ØZŸ‰@kk!ŒÏ¿Û½*,ú4?ïïÙAOU©¿ìaÏþ°t§¿ÑHdà
—¿å!){#ŒÍ¿ïÿÐ/WÜ`AGNbcuNVSS J082236-263125?ïñÞúr?^ã‰Ê»Ë?\BñŠ?^ã‰Ê»Ù?ïÙüsÀ,/?â[Ÿ>ëN?sÆéèé?â[Ÿ>ëO?ïºÄ:g?~ 6Î$LV?Nü1zf¸?~ 6Î$LX?ï™ä)zú?z|$Þ2ù?‰†øµ¡A¸?z|$Þ2ù4FGL J0823.1-6330?ͨ}ÊÀ-Y± žÛùÀ;¤öL"'À<¿';ý@"Ùa…«ü?úaAcwž?Òæ">eìC?°=˶¶¶?Ý¡faÞÂC?ý¤¬	ˆ¿Ø¿ïǃý{u¿èó.0D?æ/ùø??¾îê.£ˆ¿é²ò€»|B?Ùã&2ƒAGNbll1RXS J082316.0-632928?ïþÉ×ãg<?kO·»Ñj?#bÉŒ8Á?kO·»ÐÜ?ïü-w%?`¢E??þ"GvÛº?`¢E	?ッÀ}B?˜@f?€"àºïÂ?˜@i?ïîÞõúF?XÉM^Ç÷t?a÷!
»B?XÉM^Ç÷i4FGL J0823.1+4042¿ÐçéçIY@A
CނØÀ:K _ŠÀ<S½—¥£"@E§håÎ@Ľý&0ì?¸ÛÖÕå$]¿˜Ù·–Ú¢?ßi›"Ö>@KÖWºüì?ê_ëä¿è°Ô^;Ÿ"¿æ†Û†£ó¿çÞavؤ¿ÒB&€IR¿ïü5ۄµAGNfsrq3FGL J0822.9+4041B3 0819+408?ïýw‹4ä?1Žz_P±?4GK¦Xã2?1Žz_P²?ïþq"Øñ?B	¥0˜-H?(î¶ÂpïÕ?B	¥0˜-J?ïëkEøµb?fz¯'˜ƒ?d"ºJ?fz¯'˜v?ïÿTÉ©•?R_-r©?µfÊÍa;?R_-rA4FGL J0823.3+2224?îÒÇçaÑ&@=­gf@¦¹À:q(•J€À<rv.Z†^@yðÿ±üg@#Nƒñ'¨?Á±=òÕ?º"»¼Pí?ö4ƒzsc¥@q,/³ÌÌ?ïªì¨4g¿Æèž9'q¿åèº3mÖ¿å*@ ¯¿ã5ækÚ¿ïÿàŠï²«AGNbllOJ 233?ïäå^Ù?ih¾Æ7·?kâ¡b&Ø?ih¾Æ7·?ïó­ð·<?iƒçS?X¤ڑŠ?iƒçS?ïÚ±WXG?Š°÷
øb{?©Õ÷?Š°÷
øby?ï̋ƒ?†íÝáÒs£?ŸFnÏœu?†íÝáÒs¤4FGL J0823.7-4838?ÎÞé~È?À¤B"ßÎ1À9GÙ.ÚÞÞÀ;-‡É},@'¶iÞì@uò£ +?ÀAž0O‹?±j¿ë½Ô?ñj µ'-l@ÛW‰Ôª'?ëGU^×%ì¿éfA·/'¿è¦¶~¡Ç¿åýÃÝéU¿ìÔ
xÿÆ¿ïù·KAGNbcu3FGL J0823.6-4838PMN J0823-4837?ïÆJæ1?"F,'@5d?|ÚÿþŒçT?"F,'@5d?ŸÆ ?¡÷Éj´øö?‹Ö|Wì?¡÷Éj´øö?îŒÆ}G½|?œÂÃÿ¶ÿ?§3˜+"(D?œÂÃÿ¶ý?î>º£eë?'^Ðçü~?¬UÉ®¡W?'^Ðçü~4FGL J0824.4+2440¿àŒ.ÀûÍÆ@>¢v§&JÀ9žØ:¿¯À<û¶Å#‹@k"+'s@qý"ÕíÞ?°¢"hR#ä¿¢…>©€d?ðÑ}†=œC@!BԐæm?Âcþ"8¿åâX"ÖÅ¿çñâÀÿäý¿áÆýX…Ó¿ç¹û~»òµ¿äGDžkAGNfsrq3FGL J0824.1+2434B2 0821+24?ïü‡'ôV?3ÔÏõu£Ë?;Ãè]KñK?3ÔÏõu£²?ïý‡û¨kÝ?PÁK˜f÷(?3À"¼¡2?PÁK˜f÷/?ï湕õú?kŪ~ƒî²?iFj
å`?kŪ~ƒîš?ïÿ»'¶~>ó'ó¬ÁÄ?>'`ÕÔ>ó'ó¬À4FGL J0824.7+5552?Ä­"ëêÙ@AüPHÀ9yú Âî'À<b[ŒÐ×@ŽWáé>@ÀY+",?ªæ%®¨?ž½»"GoM?î\fhå@͘îxîÿ?³ÜÝf"â¿å˜ËЮڿç»ÉÚª"¿èœm¿ ;à¿å(œ×;»˜¿ïÿ±'#áAGNfsrq3FGL J0824.9+5551OJ 535?ïÿ,—¡Tb?×wŽ<†$?mÕsâT?×wŽ<…À?ïüîNT??M©¿ÀL•3?8^ÃV?M©¿ÀL•?ïé¡¿è?hfz¨?fí^ý@?hfz¡?ïþq¤p¤Y?%R7K'ƒ?(å¸õºh•?%R7K'Ê4FGL J0824.9+3915?ï÷®€@@A¦ÊıÀ9'ÛçòÃÀ<Q¶¯T@ü¦–WDà@öƉ¼­?±Ï	¤ïc?º@ÂèÈUð@fhÝ9+›@˜q±CÞ?î¤vlmçd¿ÝM'iÒ,¿ç–ŸV¿äq¦ ¿ç¿ëÙ~áÝU0¿ïÿÏù§÷*AGNfsrq3FGL J0824.9+39164C +39.23?ïöOÙI—?SÉ34tQ?S`MmÀÔn?SÉ34tF?ïàKeõC¡?…YRdr¶?o´š
¼]i?…YRdr¶?ïZºÚ^Ï?¾w˜"p?"¨¤´&°?¾w˜"p?ï~t(Ä@?‡F\
¤kö?ž1zçw×?‡F\
¤kõ4FGL J0825.8+0309?ÑFàMC@6c¾˜V£{À9‹¶–ç8À<>æ¾æZ=@쮪ì}@œ@WV?¯_8ÕX7¿@¢>ͨç?'i1qçú?ûA7ë~¾¢?ï7É
ûk¿äÙ¸£J"¿ãœ
!Áñ§¿ágFáúÊ¿ã‹= Êei¿ÙoÐ<ÃÕ­AGNbll3FGL J0826.0+0307PKS 0823+033?ï³x|$°'?t~`bôÀo?ƒ!àöÓöU?t~`bôÀm?ïÌ^Dl'?m‹3®ó?yÐÝÉ·}?m‹3®ó?ŽŒ4?ˆÓgD@RU?™\|Üó!?ˆÓgD@RP?î‡Ô€-î%?">çboê?§'·ý!¢?">çboê4FGL J0825.9-3218?ç«P‹t#@
tO»)6ZÀ9NW±—½!À;¦€ç,¬@"­K¨@ºZÚA*?·ì
µÂÅ?Ï£Û¼Ô²@è&grÕà@wT©¥€X¿Ù߄ÊÕ{È¿à"b*—ƒ¿éE½úL¿è5QGq¿îÐîdÍ	3¿ëÓb}£™ÎAGNbcu3FGL J0825.8-3217PKS 0823-321?ë‹@Ûòp?¿3˜Žü?ÁÒÿ¨6>?¿3˜Žü?ï;¸Æ¬_ê?¹…MˆrÙÔ?˜ˆç*tÄ?¹…MˆrÙÔ?êhv‹§ã¤?±B»Î¥?Æ^%Ñ`qm?±B»Î¥?ïœ';ŸÉ?†ä]•9w?ŸŒ{Œô?†ä]•9y4FGL J0825.9-2230?ßOÖlÓ@!ÙöD•[FÀ7ތXhvâÀ;J	{¸@Ô{Aê±?þŽ&žÐ:@?šN‹9•´?°…OŠ¬Á¿@ÿkã}é:@Í+Pæ¢a¿£ãŽZKP¿×ôsúù…è¿á¿6â]¿Û@êa2J¿äšÀá@¿åuÀ –ùVAGNbll3FGL J0825.9-2230PKS 0823-223?ïü¹'´xè?5rC
a%?:3r\8ÃÄ?5rC
a'?ïâñÇ!K?ƒ!T"Ó^?m8Þè¶3?ƒ!T"Ó\?ïÓú|S7?ñ0#Eßx?vÁðVdl?ñ0#Eß?ïñ£î"?GoHu"öÜ?\z¸"÷þw?GoHu"öá4FGL J0826.4-6404¿Üó-ä°@šÀ-XçW'Ž
À:‡‡H^>À<='JSá@!ã~êì?üqšânõ?·SÈ)$?œ(b}VK?叀[@áäÃ
±D?ëEKß&–˜¿àȳÞq!¿Ò•½Áìõ¿ßû[O¿Ø¡ŸAÏ-O¿ÌŽ9G¡AGNbll3FGL J0826.3-6400SUMSS J082627-640414?ïüS䗩"?7D¹'ä'#?=`ÛB³ê¶?7D¹'ä'?ïý՞ù'µ?L+nHcÜÜ?1S3j^U?L+nHcÜÊ?ïñ¥ó×?hÎ(ïÛgè?]Ú´ÎP©?hÎ(ïÛgá?ïë—õxäÍ?Rt6™ë?dh
‡3¡?Rt6™ç4FGL J0827.0-0708¿'}6F9ˆ@1† yKÀ:¼gú»À<5m%H{@ ®TL2ˆ"?ú݁5ž?À1xÞc"9?Ãúr¢^å@7ßÖjÛ@ûEá`­•?ïòMZ%æD?Ýêßqêþç¿ÂÑå:Ü¿Ï÷ ÞFò®¿ã™:Ü¿ÖElÜ!SAGNbll3FGL J0827.2-0711PMN J0827-0708?ïá|ãâ¬q?jÜ/PO¯?nƒSC?jÜ/PO±?ïà àº¯Ñ?…6@/)Y?o_EP/"?…6@/)X?ïª3A@ q?ƒ›_\$¹?…s/¯×ãä?ƒ›_\$º?îȈŽÂÒ?ˆË×7çjË?£ww£Òâ?ˆË×7çjÉ4FGL J0827.6-3735?àrP{n?áß®PàÃÀ9\‰Õ×7ŠÀ;-«‰†&@ŒhF]0@ì["e…–?Ì,Ë:%•¼?Îñ¬€&+
@%[Új@
±´Ãk¥¿Á«w½{Ëþ¿å`=Wyc™¿ìD‡•¿ïýÜ¿‰k?âɃ¡àø¿ï¶1J$ç@AGNbcu1FGL J0827.9-3738PKS B0826-373?ïñý÷Љp?t~en~c?\^í l?t~en~`?ïñ¤ÊI9?‡Ïåê<Æ?\¶jýmŽ?‡Ïåê<Å?ë§Î‰5ñB?ªò£´²¥?Á`ÅÛ(:þ?ªò£´²¥?ïúíNf?AÕ<úg?DK«®Æmõ?AÕ<úg4FGL J0827.8+5221¿ïÑ•çß@AÔîàóË>À;Sx›ó-À<¸[j‰á–@ ‡%["5.@µPy•T?̊›9ÖÚ¿Í¶ùôº?Àvþ#±àã@¿ñÇx?ëKå±  œ¿è	cr– ¿è]ÕÉ ¿Úm¾I|K¿ß[ÿDÄ*<¿à]¾÷÷ôAGNfsrq3FGL J0828.5+5217TXS 0824+524?ïú»ÎK³Š?BW®üA?EÆÑ1Öó?BW®üS?ïýºÂPz±?`CXõœ•?2)í|*{?`CXõœ•?ïïçQ¼y}?nª8VÁ—6?`®C†'Þ?nª8VÁ—/?ïëøy%l?Q·m4Iç?dþ†Ú"6?Q·m4Iç4FGL J0828.0+2307?ï×yþÊ@>ﯷéÀ;
ê0ŠâGÀ<Ÿ	"5"@ ü¢¥‹•?üÉJç"Þ÷?Çö·ÂN™–?¸'ˆá±O?ñØyÞé/@~ç­Î¯Ñ¿™ª8€Ø‹%?í¨ÊߌÂò¿Ø•Þ#6eî¿âHdóŸŸm¿ÉÞ¶Ö:µ¿ê³
¹—eãAGNbllNVSS J082801+231215?ïûù#$`e?Cdcލ@?@sn~m1?Cdcލ>?ïúsßÇ¡^?b]ç0óÔí?F0€áz"s?b]ç0óÔè?ïÙH9!=?uÈéÿšSŽ?s[ócoa??uÈéÿšSŠ?ïp¤»)Hß?â{*W\?'ëhšÖä(?â{*W\4FGL J0828.3+4152¿ï÷f¯—¶@A˜©Þ‹;2À;›ík¨Å‡À<â{s=å>@!6ÛìOt?ýÖ`)5ƒp?ÍW³›"…¼?˜';½'v?Ιë£ýu·?úYC[öÌ¿é|O÷Æ¿îEÌþJô?Çg_	й@¿é&b@¼ß¿¬ÖI"]Í濸%^^Z(kAGNbllB3 0824+420?ïþ¤ŒCOp?&}\3΂?%·;Ë	Þ?&}\3΂R?ïý%»‡?LP;™Ó_?3†Ò'+ºž?LP;™Ó`?ïÓ´«"Ґ?x%=cÞ
?v%ª5–·Õ?x%=cÞ?ïî«M¬-´?WYa»õ¸?aT²SÒK;?WYa»õ¶4FGL J0828.6-0747?æ*͖pÀ@1‡"%RDÀ:›ÇqC9À<l_˜ìËp@'ÖÃñ†ë@;™ÔQüL?ÔÖàâXz@?ä–ëip@µV=ú6'@èHÎÐÝþ?ïåÃ=×Ñä?>ê!¿ëÃÏ,ù]O¿âËñqÇÿå;Ðá.ƒ¡¿åIßG"ÔAGNbcuNVSS J082854-074854?î'«o «þ?²Žs¹¹?­…I
õ@?²Žs¹¹?æ7Ö®š?ÒK˜ÌMåj?ÓǑèR¢Í?ÒK˜ÌMåj?릷:'å?©/ÏKž?Áe#¶m?©/ÏKŸ?æL˜.Ñ?¸°ÿN'œU?ÓfÏÉÿ¢^?¸°ÿN'œV4FGL J0828.7-2422?å4î3‹@ ÀîIõ˜À:̹-³—rÀ<\w—|@^Ù<å@
¥³Ú?Å¢7"0?šP¥<˜•@?Ö¡ô›<@f
#‹?ïÿ€³ï†5¿ç¼"¦Ò¿æ"
q¿Öž:}ªOÊ¿åïŽÎd|¿ïÿz)5ÙAGNbll3FGL J0828.8-2420NVSS J082841-241850?ïü¿Ð!@÷?75vµžñ5?:~õøK…?75vµžñm?ïùýø;ØS?e'½ã?Hž¯?e'½ã?ïৈ7õà?t³r,UÔ?oXwÈ
?t³r,UÌ?ïÙÁ·Èð?[²Ñ"œW¥?s$‡¸*?[²Ñ"œW"4FGL J0829.0+1755?é¢Eï$@=]Ù©T"À:pÓ¥¸À<t3Øt ¼@¸ÂÒ¢ú–@7·&rZ?Á=¦©¢{?¹õeó#ù"?úo|—@‡sÐÝ'¹?ïä"pB]¿Ü•)<ºEŒ¿ãðís5Â¿ÞŒ~þã ¿ê†-vZÐ0?™BüÔÒTÌAGNbllTXS 0826+180?タ«Å0x?|jÂÒ%$?€_Õ³â/?|jÂÒ%(?ïóÁ)æÌ?ld#ǔ?X}¬3Ðhõ?ld#ǔ?ï5ƒÂšE?"Ž'ˆ?™O‡¬·NK?"Ž'†?ï
ç:;Å?…«ö¤°8?žC¸‡]q?…«ö¤°84FGL J0829.4+0857¿æýÖzA݃@9ÐÉûa4ÎÀ:ΖãܳËÀ<'ñŒŸ¶@6"1Rˆc@‰ek"¤?Á€¸HÜ=¿] "øáL?WP¸˜ý@PeAxEa?ïõ+Z÷[¿âH^=¢ø¾¿àÖCnÙÒ¿á`{jÚin¿ßò)é•ö¿ÕwyÿJxtAGNfsrq3FGL J0829.3+0901TXS 0826+091?ïõ°t%ž°?LZý¢-L?TŸ´Â ?LZý¢-[?ïþ~Ž?D)ã;÷Åd?.NÐ?D)ã;÷Åg?ïí3ôð?k-ÝÃY>r?bÌüþ˜?k-ÝÃY>O?ïáX6¶'ï?U>xðÓÞ?n§ÉI}•?U>xðÓê4FGL J0829.6-1140¿íüúí›õC@/T)¥ë·À9ÍRúxׂÀ<9KWí&ß@Åq%\0?ÿÖeÒ°?µ–È®ÚôX?²†8—·?ýÄxœÉÐ@K¬Ñ¯µ?ïÿÿÊPË¿ß±$ûŒÿ¿ãì@§Ú¿Ó¯ÎD¬¿ã‰u_'®¿éÚ~Q1AGNbcu3FGL J0829.6-1137NVSS J082939-114103?ïý' /Ý?4X«29ˆ-?6Æþƒy1?4X«29ˆ??ïâöÕö?'½h…zà'?má	ç*
É?'½h…zà%?ïá£l–>?qäØ°ŽT.?n\"iÁâ>?qäØ°ŽT%?ïd ²ÉDh?x;4¡X?"{é¦×s?x;4¡X4FGL J0829.7+5105¿ÐÏgÖ\{A@Aûd­ÿ',À;A³àl½À<ÛãÛÝ@˜¥ûý'ç?ÿµA*l»?ÎK`æõ—ò?¬øƒcø"?á!aRüQ?ûZÈΪ¿æv!ÅL¥Ë¿à…'âr%Œ¿ä¡‡¿}¿ªcÃ|t£¿ïÿ"Àh¡?ïóÕðaýKAGNbllGB6 J0829+5108?ïû°€3tŽ?@B×uòãŒ?A=ÿ2-Æä?@B×uòã‡?ïï8eÕg?he¥àìB?`bǚ*—Ç?he¥àì>?ï`Ní@—?ˆ9^_<f?Œ§ìD¯Ú`?ˆ9^_<d?ïÄ	ç™'?sÜNÃ~Šx?}ÿ{3lœ?sÜNÃ~Šx4FGL J0829.7-5856¿áÜ·=Ú3À'÷¾æÀ9Œòã·ÊÝÀ<<ʋ©í@J€×¬@€Á@§ü?µØáò½'?³HÐ(ví?ûˆ5©/8Ó@éI&÷ç¿ÔI":<'¿å§zޢ߿çÖj¥Gá¿æ¯qr3#C¿ð?ïÆ1bM§ÿAGNbcu3FGL J0830.3-5855PMN J0829-5856?ïòÚÁ§ý?j=ÿÞG'?ZKô|°=?j=ÿÞG?ï®?Ç-}?¤ã̂ñÂ?"p4 ˜©?¤ã̂ñÂ?ïU&ma`X?'FùSh
?•[2SÓôû?'FùSh
?ïeé¡ li?"_¤ŸL£?"BËËòr ?"_¤ŸL£4FGL J0830.0+5231¿ìœ·…;@Aÿz¢]zÀ;ðG%XÀ<¼•¹:I@ žBFK"?ÿƺ~ìo*?Ι>ív?~r‡î¿?ªDOÿáeû@ÍãùI¿å -à
¿ÜÜ
œö›R?îÞ!¯é¿ßu¸ÿ:ˆ<¿ìwÛ~kjÝ?ÛF.b"óèAGNbcuRX J0830.1+5230?ïø¥ÏÜ[Æ?I΁¹ç)?MhÀŽæ)?I΁¹ç?ïü:¶4gÙ?d®)8Üú ?>*N\Á=Í?d®)8Üú&?ïHÎñ8?'³sA?ÈU?–æ<ޙ?'³sA?ÈU?ïïól\ðç?YçõäŸeO?`"£?YçõäŸeI4FGL J0830.1-0946?ص™ÖRž=@0ÊFà!qÀ;A8"ÀõÀ<©!6±m@ ìcÎ[˜,?ý°áxÚ?Ìh´‰ßè3?£ý?[_¢'?Ü:…M\T@?%ƒr:Û?ïÿùSt¿èýÒ~<›è¿ßŠ'¥aMù¿â9gàd`¿©¶I¨•Šì¿àÚ¡'µ AGNbcu1RXS J083014.6-094455?ïÿÜK•W>ðµÇõI&>ñÚ5wÔ1‹>ðµÇõHê?ïýÒ"v?SmËòð×1?1nï/K"?SmËòð×1?ï÷ԑŠ©d?YIÑþ±)"?PVÜê­9W?YIÑþ±)©?ïý–­?$ÀéiËái?3J—Ï/Žb?$ÀéiËá!4FGL J0830.8+2410?à_>ÒuŽ@?ÛøvžÂÎÀ8´wcä¬À;܋Hþƒ@ÿ).L™Œ@L±:?¦SN† Ã"?À³Eý9@ù/+f¶@—Šh"¿×ÔÁû¿ã9[e¿æà›$´¿é:귙^á¿ì½Ú@¨¼¢¿ïÿïXzAGNFSRQ3FGL J0830.7+2408S3 0827+24?ïùU^÷ÊÚ?Ea¢ÿÕ?Jª" Ԛ›?Ea¢ÿÕ(?ïöà)Þ?l6ëÞ¶³?R?ÃÙ¬GL?l6ëÞ¶±?ï¥ÂÔú×?"²j$êË?†JÁJ>"?"²j$êË?ïÿ"cW¥Ô?{º¢?
ç*ŠòH?{º'4FGL J0831.4+2631¿ì-'Åt9…@@ZŒÞ 3èÀ:یwr'eÀ<r7€ŸÍ@í5eèg2@+Iº?Ê°9FÅ?¢ô¤­Ï?Öin¼ó¼@ëpõ3s¿ãà]¾!8_¿áË¿¹Ó¿ê'Úgê¿ÞØ|ßy£¿ïýĆ­-Ë¿îÍ´Þïd&AGNbcu3FGL J0830.8+2629MG2 J083121+2629?ïóáá­?YÑÄÉÎ	ý?X=ð=ð£Š?YÑÄÉÎ
?ïø_9ê?tó0Õ}ü?NƒW·µb?tó0Õ}ù?ï°QØl7'?'`ÿ^ó?ƒë‰äò¨?'`ÿ^ò?ïÚU‰<˜?c;Nsp?rÿU;a³ï?c;Nsp4FGL J0831.5+1747?îÿÉ"@=Úþ£ßm¹À:µq5ÍÀ<~ùÛ"Ðå@ ¤ßðbÿ?ü2ÑɋϬ?È	¤"ZS?ÈBY@ãö@¡³CŽË	@?Ücï(
u¤ÇË?ïãՂS?ǒ£Ì´ú¿ÝiÀ8î¿Ýïø€¯½È¿æ«œ 1£¼AGNbllGB6 J0831+1746?ïûaã ?Aí"}©]å?B{èsÅ'?Aí"}©]ù?ïúÞk}ÞÑ?Z ¥"Ê?D†R"¼?Z ¥"À?ïÍéøò?|BíKx«?y|r‹†À?|BíKx«"?ï¨á™.%É?r÷•§…¢?…Ç™´v¡?r÷•§…¤4FGL J0831.8+0429?æzf©Kî³@8YVŸIÀ8,vü¶ŸdÀ;«UãTÏ@yïJ%=&@rN¨Ú?-ÞM?³{1yŸ©(@ÃÉîËû@;ț9×½¿È••~Å¿ß4ä"ÔÁ8¿å$ŽTÁù¿ãŸLa¢—¿èþ5$¤û¿éáä¡ÂAGNbll3FGL J0831.9+0430PKS 0829+046?ïü¿Ë§"B?4ø~<.?:¢Æíé¡?4ø~<??ïõ(ò=ö?k/	"PœÜ?U®"æé?k/	"PœÜ?ïç篩̈?kJÛµºËë?hPV3wM?kJÛµºËñ?ïûØÅ5¨™?0à³ÏÚ`?@œë)] P?0à³Ïڅ4FGL J0832.2+2753?ÚÆp8@@ ì•¿ðEÀ;8^B«v;À<¨PŸTÄ}@"Ô¿Šo@'™Ù;?П‹€Ò"w?¿_ë^C"d?ìv¥CÃ?ø3 Ä̊?ïñ`®–¿äë‰>ÿàK08¬ð¿å՟¿MˆI¿êg+R"!‹¿¶‡ä‰ŠÙAGNbcuOJ 250?ïÛitLòQ?p2åæëÃ?rKEنÖÅ?p2åæëÃ?ï= Ö£ÔÒ?©ž±p³'?˜Kå+…eï?©ž±p³'?ïXÀò "?2~CÊ¡?"çá®[í™?2~Cʤ?íȶëŒC5?—3œ¥?±ºH£æ_?—3œ¥4FGL J0832.4+4912?ì݉[ޖ@B1yЦv!À:A0«™v^À<˜Ç¤nß²@¾]r¡Þ@¾\ǁ3?µõÞ;¿ŠS‡;žÍ?ԘÂÚô?÷÷/™Ë˜š¿ßÞ¿þÞ÷¿ãc-ÌÁå¿æ®x?'æ¿ãU1Š¼‡¿å%yœÝò¿äF="†AGNbll3FGL J0832.6+4914OJ 448?ïÎø',r/?rá'Nàw?xƒ·iÆçÉ?rá'Nà{?ï©–	.ï?˜êwu?…¾Z}´D'?˜êwu?ïø·÷C?‡þb‹9?Ò?Â/?‡þb‹3?î•_`¦2?'•Ž+/aÄ?¦®ú	õœØ?'•Ž+/aÄ4FGL J0833.4-0458¿ìÏÉFº@4+"Ù@yÀ;çÌ,"ÝÀ<èj±NÂ@¦9$¹È¹?ú6çÚ+?Ôö+ÀÎð?åÞN4@ym@››]@'~ã	û?ﮔ"6`º?ְߛÜiù? +€À"À¿àvH¿ïÿ­?å`¿È~£®$kAGNfsrqPMN J0833-0454?Ö "~?Ëø<Û\]Î?äïùîþ@ò?Ëø<Û\]Î?á:K˜¥:õ?Ù
"UÍ¡?݋hεŠ?Ù
"UÍ¡?Ñø†^g?³Ù©oe?çqƒó¼ÐÍ?³Ù©oeŽ?ßáòÎÄÕ?¶Ñøì5?à˜ý•?¶Ñøì54FGL J0833.9+4223¿ì»2Õ5O@B"ÂÎFIÀ9Û‡\€4À<uJïèZÈ@#S—+Ö@<A<
rJ?³ìhžyþ?¥z{TDP?ðœí¬@eK@
U€ºûi?ïþ,‹yEf¿âϕ¿ol¿ç'K³žÓ¿àmš7NJç¿í§VPn­]¿ïñÍ!ÜHÁAGNfsrq3FGL J0834.1+4223OJ 451?ïù"ÑœAt?F•úL?I칎ú'û?F•ú`?ïúTéÄúö?`É]17ûa?F¬Xì'Î?`É]17û[?ïÆ}­›¶?~Cï¼øã?|Á)29$@?~Cï¼øé?$r-á?nfÕÉ·?€Þã{tˆ(?nfÕÉÂÀ4FGL J0834.6+4402?é\?jv¿@BFK†ýÀ:yÞfRDÀ<§—L¸?w@Ý(bŸ²b@CF uÁM?¿iS֖Ð?½§Žú¯34?üK‡mG+8@	E…a~J3?ﭓK¡¿¿s?|0–åy¿äO›HÆBo¿ãð`̞¿á²¬ÅÆHN¿ïü:]Éß³AGNbll3FGL J0834.7+4403B3 0831+442?ïøÓ³A»?P\×Ü£Ì?L±3Òù˜?P\×Ü£Ì?ïûˆ˜ÑZÒ?VëQã'b?Aݜº"·—?VëQã'R?ïÈO[Z)?zÔ]ý½?{Ø{ÒRë?zÔ]ý½?ïÃÿ¤M?eµöà¡1?~-üðXË?eµöà¡04FGL J0835.0+6243¿ìÁÅ£çÀ@AÙGNΚÀ:ê"@lÚÀ<ˆ$GÝå#@SÒ¾SbS@<=3g6?øŠØ¡e?¬À'¤)añ?Ø9ºáè¾?úu…•Ö–z?ïþÛ½«q³¿èÝ¡ÜF¿ífÒ1›Ä¿êŸ—£ö¿ïJ˜ñÓí¿ÞÃÓߐžÉAGNbcuGB6 J0834+6249?ïú.ª¬m°?Wîçfù·?GEUNI8ê?Wîçfù¶ù?íÞ[%´þõ?¿w/eâ?±
&ÒX[?¿w/eâ?î9>;~ÛÏ?¡(߃‰w?¬lHC?¡(߃‰v?ígE;ª?¶c'KÜ?´ÅÖ'ßR«?¶c'KÜ4FGL J0835.2-2243?íå` ï‹@%›™N?À;>ŒjÜí¬À<߄ۜsi@@'I}"@	ۛœ©?Ö £ylS?ïÿülò@ÿ3å	Út?ÿ4]q +?ïñô¿Zƒ¿á½Zi¿àøú'0?¿íÔ-ê¿ïîÌț¿ííËJÍÈAGNfsrqPMN J0834-2241	?âd›­[ô?ҔÀ"tøé?Û6ÉØ¥H?ҔÀ"tøê?Áã@²ôÏr?ÍQ(÷¾üv?ë‡/ÓBÌ"?ÍQ(÷¾üv?ÙL)`àu&?¸éM'öŠ?ãYëOÅm?¸éM'öŠ?˜@OÏäÂ.?ƒüD"x?ï=ý€Ùï?ƒüD"y4FGL J0835.7+0936¿é T5w¾(@;"È6eÛÀ:ÛÉÃ-ÚÀ<Š€Þ·°Ü@Êõ7O!¦@·{¿"ÿ&?ȂÛgj?¦"¶]Ÿ˜?ã—ñ=Å]m@ ÄÃéÏ<?ïûB0&8¿Á%l5³@4¿ç¾"7Z	¿ß@\[˂˿ål¯UÀô¿àÍÛÀ…—AGNbll3FGL J0835.4+0930GB6 J0835+0936?ïúö­››µ?Bñ'íñœ?D%I''.Ó?Bñ'íñ©?ïý9×O?WP:´GÊ?67éE‡Ì?WP:´GÄ?ïìλ"%a?j®»Þê¢S?c1DÝڞ%?j®»Þê¢L?ïé¢"ú?Pp}g>$§?f=]ê{¹?Pp}g>$®4FGL J0836.2+2141¿âåà1H-:@@'óUÎÀ:+?› 'À<b¶FxŠU@ìõ[â(ÿ@ö+ —ºœ?¹|ZÞr習"¼\‰/?Ôg˜*-Ðô@	õ½©Ä4"?¿É읢'½¿æ©ÛÑLŽN¿ébÇ«$ÜX¿å<÷‡¿ïtRQÜl¿íoÙ¬¯ AGNbcu3FGL J0836.3+2143MG2 J083615+2138?ïùkžÆw€?HÍwçÍ?JQ"æ!þÊ?HÍwçÊ?ïý)j=¥Õ?aG…Ü,âÞ?6´®Ñdä?aG…Ü,âã?ïã‰êú¤?nîìÈ7Bú?lvïYÕ?nîìÈ7Bþ?ïí©kÐO=?TkKh6k"?bV"/°ÃH?TkKh6k4FGL J0836.5-2026?ËyÖê–@(9	(­ûÀ9ÞØ-SbÀ<&æ"Gp@rxJ"xÈ@¢|—*T?Ã([!?Ò7ö{ò¿¦@)È»ÆL@	ÒÀº컿ÝÑK·Žw¿ãŒk'fL¿ìæMÂ*²[¿ïÞï@4£¿ð?ïÿþBe«+AGNfsrq3FGL J0836.5-2020PKS 0834-20?ïû4/¡æ?H5áîæ—?C/Cýxd¯?H5áîæ?î=F·y"´?Á}V*	ƒ?¬+"ˆmÔ¸?Á}V*	ƒ?íA"vÕ?¢ÙêÊzM?µóßIW|?¢ÙêÊzJ?ïz9Qã?†k¼£½?¸ÝUݞ?†k¼£½4FGL J0836.9+5833?à_ÙL~@BDaAcwŸÀ:ÆWꢠ©À<¦­@?‹0@¡¸Ðìl$@º:Þù;?¸a.n'z³íPÑ?ñ–¿Ê…Ë?ýq
×tp•¿ÜÏ|¿ïÒ¿áN
>¬ãù¿çh?ŸR@?¿âj4¼ .ß¿ã"2þ¿Ø­JÜKAGNbllNVSS J083705+583151?ïÞ:"ƒ3¯?gC·3Ÿë´?pâµ¾f('?gC·3Ÿë²?ïáZ™Àgw?ƒS!yåèÒ?n¥f?˜ˆí?ƒS!yåèÓ?ïÆWôâ?yó$HÄR·?|Ôýx¸?yó$HÄR§?ïB%R3‡?€8QdÈÊ?—»U¹ï:?€8QdÈÊ4FGL J0837.3+1458¿ï"Y4€@>ȼœÓáÀ;)(Fp&ÚÀ<§p¶K@ ö
³\Z?ú'¢ê{3}?ÖÒ"4ÕË?Áéoo¦V?ñ¢.x¹OB?ý1D‹u>›¿ï±E½yr³?ï;ˆÂ0ç~¿éT•]õ©?5n&NHbo¿ÞëF'¿àª|uœdOAGNbllRGB J0837+149?ïûj8‡Ú?CÏÜ!XB ?BWà—ö[?CÏÜ!XB
?ïúm^f\J?[¶E˜Ûr?FJ†fŽÔý?[¶E˜Ûqô?ïÌÅ@^[?|§Úœæ4ž?y_õPÒ?|§Úœæ4Ÿ?匿àVßî?s9*J[V¢?†êHg?s9*J[V£4FGL J0839.4+1803?îõZ uº@?¶·ª%ÙÀ:`þU/ÝÀ<€VAU5@ùZ<a…@Ž±=û
R?¶Ðó-‰¦¿œ܃yË?å±
õ´M@»<.Y"¬¿ËßÀ‹t¿ÞZ~¦¤¿ä	`0Â?«¿åJŸb0w¿á•`Nõ1¿ÌBEÈa-AGNbll3FGL J0839.6+1803TXS 0836+182?ïürMû?6š°Ž…"??÷ìm,¶?6š°Ž…?ïýÆ·°'?GMÿœym?1ÊG2{p?GMÿœyt?ïðPwÁÛç?f»PŒoÂÓ?__|H1›?f»PŒoÂ×?ïöâ…í?@S«DI?SùÊ:ô(?@S«DI‡4FGL J0839.7+3540?ÄKÛÂÆ]q@BA,üœÀ:RÆvqvÀ<ozLÍ8-@ãÿ:³/B?þ¬€&+
?ºÛâ~å¹-?¶$[T ?ü§‡H^=£@çV:õ?ïþ7+æ8¿â¨Oªb>¹¿ÙÀ[¥B¿ÝP»>Z¿álšÈmÂ{¿â	P
ÚN–AGNbll3FGL J0839.6+3538NVSS J083943+354001?ïö°²öV?PxÞ
T¥?Rž›ÖSÀ?PxÞ
Tª?ïö*¶Û?h7Uæ2?Sª"îIS?h7Uæ:?ïÑ)ŵÝ)?z™
÷÷+?wk%jÐ?z™
÷÷?ï&õî6w
?~cÔ''?›!B91o?~cÔ'~4FGL J0839.8+0105?ÙphJ{ì@8uà'Œ6ÛÀ9™'ÿùJÀ<Êþì@æAzɟÇ@î][$éÄ?µŽOŸ¶¥T?ȟ©érõÁ@ÂÇut÷#@~‹ž":¿ÓÐÂÛ\\¢¿à"0±x³p¿äSø:8àò¿æýNª‡þg¿ïþôx
¿ášXÜ:(AGNfsrq3FGL J0839.5+0102PKS 0837+012?ïx#¥3ß?•2X2ŽüN?ûŸËY"O?•2X2ŽüM?ï÷{îä?b÷'ÕÓ¸?Q	#ò7Ÿ?b÷'ÕÓ¼?ì'ôñ?¨2ǼÂ?¿›w [ðn?¨2ǼÂ?ïÙGe˜?_3ná—à?s\{Í3ýä?_3ná—ç4FGL J0840.8+1317?ç¾:"n—@>10ߛÜjÀ:"ÒÊ<ϔÀ<s¿T>E¶@¼è7"î@ᶃµ+Æ?ǜvXKñp?е£»[‹A@9E'Á@ÚEÚ)ו?Å?ïÚê¿áGïþU0¿èŒoz^Ù¿ä0|ŸÏ¿ð¿ïù^Æ^ô'AGNssrq3FGL J0840.8+13153C 207?ïè2›ìc§?k¨¡Tœ;H?gÍdœXÁ?k¨¡Tœ;F?ïüüf¡â?P–$-"©?8Êðïyk?P–$-"º?¾´M†?–©öSjl?¦E´»'ˆ?–©öSji?ïïzÐϘc?K¨ÀñŒóì?`…/0g›S?K¨ÀñŒô4FGL J0841.3-3554?çˆè>Ç_;@
î¦]¨À9ÃOu‰À;š$ˑc@ X¢õãÇe?øáS½vd?´kë
¥u?Ê:
Âá@d¼~ ïÏ@áé{Vw¿îHPÑ©«?ș5[+ŸÁ¿Ì}†éh¹Ó¿ÆÀUÛ~ÁQ¿Þâ›ìK¿çÏ,ù]OAGNbll3FGL J0841.3-3554NVSS J084121-355506?ì½­ÞR#?¹pS?º'
ofè?¹pS?î@FÃ2²?¿›hƒk\Õ?«û"ÌÞÕ?¿›hƒk\Õ?ë0*雰?®õvóÀˆ?ÃÇ?TY'=?®õvóÀˆ?íÝâZU<½?–~þö£?±í-V?–~þö£4FGL J0841.3+7053?â??€È@A6T´:çÀ7ÃÜ«g!wÀ;ÁˆÛt´@±'!PÔ@2R¯')?"r×
•ž?͛¿«Q'@,2'1ìV@ Aa*½Bì¿Ô'Õ…-%þ¿å¦BWéK¿ëƇÙ}µ8¿íTÞ긿íäÓôß:Ž¿ïï ×{|xAGNFSRQ3FGL J0841.4+70534C +71.07?ëÙaí‡Á?¿ögäXó?À›ŠxIàû?¿ögäXò?ìú.†çoÊ?Ëýj2Y§î?¸.‹Èā¸?Ëýj2Y§î?è,ᬱ‰y?¶àbƒ&?ÏLyM9Ú ?¶àbƒ'?ä̐åü?ÆãkˆNœS?ÖgÜßü4?ÆãkˆNœS4FGL J0842.3-6053?í1_Β*4À&µÅäêÑÀ9P—2·qÀ<§z¡‡@*#ô&@ºÚâ9Eœ?±j=¶nçi?¸HçÐ^QÅ@1düÙÚÒ@U"–Ó?ïm­íät‰¿à/Z`ž¦I¿åt"狕¿â"ӟNå@¿åbUË
¯ì¿ïÿÑÜ×AGNbcu3FGL J0842.0-6055PMN J0842-6053?ïý|8Š'?2"	`…ÄQ?4~;®Ô
?2"	`…Äg?ïúü"ËYø?\f—ªFÎr?DtҘ%?\f—ªFÎq?ïÌDV	1þ?x•.<SB?yÝÔûgr?x•.<S;?ïçÕ"IƒÑ?S-ûŒ‹?h*ݶ|/l?S-ûŒŽ4FGL J0842.5+0251¿éóú4{C@9é™þCg^À;$r[UÀ<©F<û3@ @Öí7%†?þJÅ 0!?Ó͝aûÁ?¹%OšÇìé?á8À ý@VJyö¼
?ï')}§ËŒ¿ïH_	B?Þs[Ao6¿ßf'd@ò9¿ââÒÞßM¿Òä\Xp"AGNbll1FGL J0842.2+0251NVSS J084225+025251?ïÿwo/+¯?
{•áªUV?Š8@?
{•áªSQ?ïþ"KÂd@?DW€)€¥
?&»CÙ¼"?DW€)€¥?ï÷KиCØ?\ӗJ"
?Qh^xP"?\ӗJ"Þ?ïð?'	þ"?LÎ2?_€Ûì¼Ã?LÎ2ù4FGL J0842.7+6656¿ì>úzÔØY@AÎa(9.À;]u&ÊÀ<›ÚGÓ
@!®â‹ÐÙ!?ÿ`›KJ.?¼_ÿ™þ™N¿¯ž
œ µ?ðçáuÑ@\.Ìò¡¿â%NÂR ¿è8BÒ§®¿Å›
bE'¿æ½™Þ¸Ý'¿Ð'xB±ÖQ?ŒâèÂAGNbllTXS 0838+671?ïýö‰ç—8?/'ÎdÓÎ?0K°ÃFL×?/'ÎdÓ¿?ïýܒV©^?G¶oŸƒÏ?1mJµ	ä?G¶oŸƒÈ?ïë Jû¹D?nîÁÍ^G?dßµF»µ?nîÁÍ^E?ïîâ‹?Tø¼ãµö?aäôäs3?Tø¼ãµú4FGL J0843.0-0853¿ã[€¦v^@3ó)¡¹ù‹À:æž&Ç&À<ƒZ­ËÆ@0]^*Ü@^/æw˜¾?Ò'Y
]Q?ßëSàý±F@p¬bÉù´@	Jod綿Î<x{í?ßÅí οæµùìÀˆ¿ëÇ(}͋9¿£ CX´¿ïýè˜Û-¹AGNbcuPMN J0843-0848?ï±<ys"?‡~™gI­?ƒ°á£9·W?‡~™gI¬?ïø[pi݀?aZ¹V™)?N'>X‰ül?aZ¹V™(?ìéêS* ?¥^è¨z´?¸°«•f¯?¥^è¨z³?ïËi¾Û²~?p]?¯ÄÚ8?zK '&Àï?p]?¯ÄÚ64FGL J0844.2+5312¿½[Ú@_@C÷…À9v}¾qÀ7À<QU>S"@×Àvþ?ÿðU2a|?ªß™ƒX?£¬Ð6f?ö²³"&k@NFæ™Q ?ï®Ê榓¿ßM™æÆs¿ãN4 C€¿Ö ËQ¢Š¿ä¹ø´²#Ô¿é6ÈééAGNbll3FGL J0843.9+5311NVSS J084411+531250?ïþ¿(¹i?&W—Ö3ï3?.
titú?&W—Ö3ï€?ïýMPšô¤?LŽ}ŒÓ?5•{(ZՎ?LŽ}ŒÓ?ïöWm¯®r?`]Vº"0?SQ$ £I?`]Vº"A?ïõÜGMÐÜ?AVw &e÷?TGqd^GÜ?AVw &e÷4FGL J0844.9-5458¿á+€(LrmÀÿ«–òmÀ8Û}½›¢À;›ñþµ}%@|"©¶Æ@7G"ê?©b}=µÌ?¸?ëÓME@§,å;Xœ@¼ÓüìÐ"?èJB1}ѿڅ]à0¿áT¬?8¥
¿Þ_œ}y¨c¿äñÿ¦™¿é̪ÍÛÁAGNbll3FGL J0845.1-5458PMN J0845-5458?ïÏlü‹£ ?tø´ìM-ß?xIº.0?tø´ìM-à?íŽq³†z?ÁÌ.L) <?³ŒrcÌ/?ÁÌ.L) ;?îߋ&ðh9?š"C÷å¹?¢Mù|}?š"C÷å¹	?êÑ"7¾ƒ?¡_''—À?nj»w!ö?¡_''—À4FGL J0845.4+0442¿æ>{Â@;lÁ"tŸÀ;OsۙïÀ<§7T*@NI.B^?ÿj`':O‡?Ϫ÷¥h"Ï?ÌûÊ;M?üÿ¦sœ¯Ï@¿P¸TE¿ïÿVø4Y¤?ïõ–àVÂZ¿áúØC""¿ßIMì¿æ¨ëÎE¿ïýøScTcAGNbcuMG1 J084516+0439?ïú¹A4\—?J»`-o?Eû.¦'?J»`-}?ïø§‹äLš?q—xœ¸Æ?MaÐn͖?q—xœ¸Ã?ï´
¼C?}º
¿=b?'ýPý<ox?}º
¿=i?ï'1p]ÅÞ?wü1ʚ¾?‹³£èŽˆÊ?wü1ʚ¾#4FGL J0845.7-5556¿ïœqºŠ]ƒÀ !¼jfÀ:‡;©À<#ú±¦@N§¯ÜÑþ@OIc÷ ]?·hã²°¿†–]¶$ÐÖ?Ï$ô×è?èE`üçi(?ïö€[¯ÿ¿à[7¹ª±¿æ÷a€£~u¿ãtUªV€¿ã}éµí¸¿ÕÁ›ì/>AGNfsrqPMN J0845-5555?ïÒíàÖ11?zSåUå?v‰"çgM?zSåUå?íùÓÞã_?»m‰¿ñèì?°3ñaäÿ?»m‰¿ñèë?ï8è?=ÿ<?èƒãI{?˜âø@R?èƒãIy?æž¡i â?´×†Zfý?ÒÃÖ½-¾<?´×†Zfý4FGL J0846.5-2609?'ê•JîŽ>@%(:û~'À:ž>Ü´¡]À<)›ûs©@"	ªÎ @jÀÒÄ?ыì\ßÿÚ?Þ&S0/@K}\L11@Àíñ_©?¡©³m¿Ù™·@ôfð¿âm5Þ^s¿ë?nu(¡	¿ïÿöût€?ì.¾ù¥sAGNbcuTXS 0844-259?è2š!IŒÍ?Æ~¨Å'¹g?Ï5—zÙÌÍ?Æ~¨Å'¹h?ÚÒ-¦ïe?ÓA_V<ò?â–÷é,ˆN?ÓA_V<ò?â0òÏ
˜?¹·™†÷`?۞aêÏÉ?¹·™†÷`?܃ܫn?ºù ©=¤¶?áÀ>ªrI?ºù ©=¤¶4FGL J0846.9+4608¿ÒÊ®ar$t@Ce]€ä–îÀ:Ò}qDçÀ<–¦¾EJ@	8NÐóx@Ü{£åLö?ЩoÐrt?Á–ÌR֒?ë¹óêH@qð]J´¿Ö,DA"Š¿â݀y7$¿èÌOÏK,N¿éàkB"#¿ïÿÛ¢¨‹û?ÈXp™ñaAGNfsrqWISE J084734.29+460928.0?ïý+ñ?:ƒ¶h±?7†§×t‰?:ƒ¶hÜ?ïôøJ‰îÂ?}kêá?Vjì"zÏ?}kêå?ïÊ¡ôœ?{åxAY?zð/±¹œ?{åxAQ?ïÜqºLYº?`‰P8æ¹?qÇ"ÙÓ"Û?`‰P8æ¹4FGL J0847.0-2336¿íSu̕ç@(hïܜM©À9×u;À;Þv˜Ñ @©lut ?ÿ
ÈÅ×F?§øä?'›Ú¶š?ì[?pé!@ƒÃŽ?ïÔv_î¿ÓŠ¬–Ì_À¿áGOµIùH¿Ý¹IbI¡4¿ÙËÿ€>T¿âØÄL0ZAGNbcu3FGL J0846.9-2336PMN J0847-2337?ïöq<ãʑ?O2"S©­?S†8jÜ_?O2"S©­?ïðûæv–=?{h®ƒ_?^3ӈ~?{h®ƒ\?ïÐ8gúß?|õóà T?wã̐|¦?|õóà L?ï¤ë*P$ú?sФpY?†Å5köÁ‡?sФpX4FGL J0847.2+1134¿Ð%Pʺèì@>æãK"SÀ9꣩½ÔÀ<#¥©rU@ þy{Añ?û4<G®ë?´Å"Z‰?£"ö>,­Õ?ò7g«
f@ÀÞöÅð¿ï½µ¢ä›ö?ïþi'jÑ/¿×JC˜e¿Ü¯ÎD¬¿ÝXÏå[?ŸÐňhwkAGNbll3FGL J0847.1+1134RX J0847.1+1133?ïþìџH?( ¬,|š?/2æ|:?( ¬,|š?ïüàÔ">Ã?S3>þ£?8ù^î	à?S3>þ§?ïíSNYµÙ?holØFÂ%?b¬±¦J'°?holØFÂ%?ïݹª
­?b˜ÿî'?q#*ôy)©?b˜ÿî'4FGL J0847.9-0702?Ó\ÁØBI@5ø`»+º™À:xºüÀ°À<dÂI¼´@úc"9:ß@°;#Â|è?¶ù¥rë¯ç? @½+ç\?çÏAò×s@ÁÔÜ:Óæ?Í>^!"¿×¦Gݏ<ɿ凾s˜©¿áè<à8Ï¿ä ©¡Nš¿âÎ÷IxAGNbll3FGL J0846.7-0651TXS 0845-068?ï¯W?µ?{#¤Ø?"9*0:"?{#¤Ø
?ïûTX»?\'þáö1?B®Ÿ'á?\'þáö%?ï´X\ÕÝ?ƒ÷¢Âã{b?'éèúʈô?ƒ÷¢Âã{a?ï´Öfœ¤Ö?iüÎóá?'ÊfXÖÊ(?iüÎóá4FGL J0848.0-0524?ïG>úá¨@6ÛíúCþ]À:À›f"À<cþë-
$@5?Ìt@3i3 @}?ƀB¸â4?¿v
xc"ù?ô¢ŸÒ˜¾¨@Ô
UÓò?ï-©¼&Œ\¿é¥Œ#Wô¿æOÿAi+é¿ï*Ú~çÆ¿ï¡3Œ†Ô¿åT/aíZâAGNfsrqPKS 0845-051?ïûŸIþˆ?E÷µ`oÉü?Aƒ¶ØÜ^?E÷µ`oÊ?ï$:ú»%?©5aƒa1?›x½¨›g?©5aƒa1?礼w²û´?"ŸÃñ³ T?…ÙâA¶?"ŸÃñ³ V?îØáò‹.v?ŽÞ£%®-?¢qà×M?ŽÞ£%®-4FGL J0848.7+0508¿æy
ÆÃå@<Zþ`Ï6À;U$H¸À<xæÞÆÊT@"øàå³x"?ù·Ab ß?ÙC«QÎ?Á"¼:-x^?ð:CȬ¬œ@ߢ8y™¿ã^V݇Z'?ïƒ}ÎaøC¿èåÛ&+ã´¿á:À›;/¿Ë¡£é©§Y?ÉqŸÕrã¢AGNbll1FGL J0848.6+0504SDSS J084839.66+050617.8?ïûñݛ'?Br_Ä5‹?@8‰"á»c?Br_Ä5y?ïü˜áñsJ?U®ØùVçÍ?;8ðte©<?U®ØùVçÈ?ïÍLš‡1­?}qEî×Ú?yY²¼g)Æ?}qEî×Ø?ïà¢ð¢?kZÂ<ٌö?o]ïì\¬?kZÂ<ٌó4FGL J0848.7+7017?ìg—®Eg@A—Ô{í·(À:£`ó_ލÀ<½ùŸ"®ž@ 
ÜkÒ6?ýDãü";?ŞÜÏyOw?ÍvBýU«®@ÄÛÄ·T–?ÿȃßÈýà?•¬g@o˄¿æŒKgÝ^ë¿Ø'(üùe\¿×m›¤`Çì¿âƁY0ô¿ïÿxPsµÚAGNbll3FGL J0848.5+7018GB6 J0848+7017?ïs˜‡Ì%ò?'‡à4sÇ?'Œï{A¨?'‡à4sÇ?ï‹/«kµ?žKe$eÀ³?4%??žKe$eÀ²?îoêõ›Òà?a>¡ܧ?©P¦BÑð?a>¡ܧ?ìzÅu]þ?ž}Èяé?¼)×ÜU?ž}Èяê4FGL J0848.9+0205?äMˆÕ@:îU7«À;(&x9́À<'IÅEïÎ@sñÀ¢@"ę?ÔÀü§…ë?Ån"›þ£´?ó?ª¥Z—ü?íqlŠ†·?ïøgºú<r?Պt";¿¿åüfîK¢–¿àÇ&/>±ì¿ïè5sS¿çåÇ°å;AGNbllPMN J0849+0206?ïyþZ•×¸?•W®œ…Ó?À4­E	#?•W®œ…Ó
?éç»Ob?εÜrKÃe?ÈcóÑÂr?εÜrKÃe?íú™ú¨"7?žD•KV?°+0*»^M?žD•KV?Üþ%:lK»?¹€Æ¼èÉ×?á€íbÉÚ#?¹€Æ¼èÉ×4FGL J0849.1+6607¿Òэ{Ó½£@B7•=êFZÀ9î.C	jÀ<}Œ†‹ŸÜ@qd<ëmÍ?þӀ*\ÊÜ?³7çßï?£Ê© ¼'\?ñpÄÃéÏ<@	B6n&#U?ïýå^0´¿ß¿ziR©ñ¿â"~§¥Ì¿×™ÒduÄ¿á‡.'ŸW¿Ý×åÐDAGNbll3FGL J0849.1+6607GB6 J0848+6605?ïþæÎhr?+vÀ¾¹?!"xÞ¤?+vÀ¿ö?ïü½2\¤þ?Oƒ¤2D?:m×þ[?Oƒ¤2>?ïõž'JÎÊ?h31rxù?TÂÛjbn…?h31rxí?ïçòSû?PÿÝœìÚ?h
¬þú®?PÿÝœìÚ4FGL J0849.4-2911?ÓX(Íz@"nf¼˜¢À:¼i¨:FÀ<=MéDÓ@Ï`¾1@heD'w?»@DÔn?³ëÉ(]±?ú
üÈ=@|U\'ô?ïþ!8^ì¿åt ñ|¯~¿ß¢ûB+¿ÞžÔw
þ¿àG†Â&€¿ëˆô›GïƒAGNbcu3FGL J0849.5-2912NVSS J084922-291149?ïþn'xÄ?'0S7ñ½?)Øs¯þ?'0S7ñ½?ïûFG…pó?`IüJ«Öˆ?Bæáê<,`?`IüJ«Ö'?ïìƒANŒË?mõü´<œ?c|¾±s4é?mõü´<"?ïòµj‰¡?BWÏoFt%?Z•*쾐?BWÏoFt%4FGL J0849.5+0456¿ì5ùø["›@<pÊ>}QÀ9×KÞ$ãåÀ<#)è0Öb@‹v9@îš|îh?¸æg¨…ŧ?¼ªŠ,¿%Å@ዻŠ…*@ÜÁ]Wõ?î™dÀsøö¿ßÈy`¿'¿ß"C")m¿ÙDÜޒȿéA¢a¿7¹¿Ûlk"¸¼ AGNbll3FGL J0849.3+0458TXS 0846+051?ï!Ñ3Zœ?˜w½{0Q?›Åٔ¬?˜w½{0O?ŠÅ̎?Ÿ. «ø?‡ÙNŒÜŒ?Ÿ. «ø?íþŒ+E¨6?¢Ê#sGñ?°ž¥Ò¾R?¢Ê#sGô?ìàZ3l%Ž?˜:ØVŽ…
?¸ý.džÓŒ?˜:ØVŽ…4FGL J0849.8-3541?ï¢Úúg;@ßãß8	\À9"8½¶¯TÀ;ºƒDÃ~o@X®ýÙà@eø5/?·;F}ù}?ĺ…aÿ#Œ@	ÂJ'k~Ô@Ž–±1ç?é¯,ÅÇ¿á–kðL¿àÈÔ_"8¿åþ†]§¥÷¿ë]Ñ6¾Øî¿Ì[ª
U‹AGNbcu3FGL J0849.9-3540PMN J0849-3541?ïц \×?rݽef}?w<¯Ñ"uÁ?rݽef}?ïôrìc!?"Ç´JŠj^?WÄ'9½$?"Ç´JŠj_?찏và^ô?¦€˜=%?º{"Hý^?¦€˜=(?ïðÂú
?Lw= ¢î?_Æz
Åê·?Lw= ¢æ4FGL J0850.0+4855?åØ^Z'¨Í@C¢õ#-+²À8¬ß½jY:À;åùɅ°@ðI°ù½@Ê]†ÃÔ?¢E!Œ¡?«}~o`z@¤ûÍkX@?X@]é?³­L¿KYñ¿ß^y½±%ý¿ãI_à:gÛ¿ãú*~å8¿å±öQo^¿å8!WnAGNbll3FGL J0850.0+4855GB6 J0850+4855?ïüJýNދ??_<¨lj?=¨‰¬µ??_<¨l?ïú\»••<?^æw2úý?F©«Í?^æw2ú?ïÛU(@"+?so¶•ãcD?rUk߶j?so¶•ãc;?ïÿ¹…û?ðÏ4è?¨Þ@ª"?ðÏ4"4FGL J0850.0+5108¿Üþ‡FÉ@C'û îÙÀ8¼$>úèÀ;üyx'â@æzšÆë@IzŘûå?¢ïÁÄ[D?µC;&x@¸ÁƒÃn@§,_›–¿Üo1CD¿Ý<+)yv¿ä0usI¤¿äûR@ê€è¿æ†é"¬ðŽ¿æðc?jyAGNNLSY13FGL J0849.9+5108SBS 0846+513?ïýÜ'ÓìK?)µ?Ì…"?1Á`ª†?)µ?Ì…?ïúL
õ'?ZÆÅ	ìӅ?FÏËø)µ-?ZÆÅ	ìӎ?ïÐeRqR?~$ÜgN1µ?wÍVÇ{Öâ?~$ÜgN1­?ïÿã¸É½v>䟡–ó¥ï>ìG6B‰jë>䟡–ó¨}4FGL J0850.1-1212?ïË_ržcS@3‡U¼Ê÷
À8w1ÅÀ;Ê+"Ù@y@¹åCç
'@<†™Õ?£3ìk£'?¶tJՑA†@pO'RÑ@ßSŽê"¿ÓW‰ÿ¯~¿àæ¯â[Te¿ã‰»€Hj¿åãZb¢®¿éêk
•ù¿äna|òšAGNfsrq3FGL J0850.2-1214PMN J0850-1213?ïüÂÙ™s?2ÇÃP;?9é7£4`ñ?2ÇÃP$?ïïã/ùt³?x±Þ<F¤©?`ЋMÒ?x±Þ<F¤¬?ï—S¿Èä ?ˆàµ…ír?Š+
Æ×ì?ˆàµ…ív?ïÿ^SaÓá?ړ˜ŒPý?5"Å"
'?ړ˜ŒO¼4FGL J0850.5+3455?ïúk²†ÐW@CHå£]gºÀ:RLƂ/ñÀ<‰I÷šÖ°@ê3ß*b@M~ˆœT?¶ç\20¿"_! í)?Þìì\µ½@[œúø\?ïý!ÿ.Hé¿âP_("ƒˆ¿àö¾È'L¿Þ¨,"mb"¿à"Ã`èM1¿Ò|Óz»ÝçAGNbll3FGL J0850.2+3500RX J0850.5+3455?ïüѪx8"?7+½
÷öù?9r¬>;eò?7+½
÷÷I?ïþ3¤V?Er¥/ØJk?,źž.Úã?Er¥/ØJZ?ïóm•7?hìŽCàp?Y%ÔÕ˒´?hìŽCà|?ïév"ú?QIO¨Yà?fæ‰kj?QIO¨Yå4FGL J0851.5+5528?Í#wcY.@CsàâiÀ9ÜE ›€úÀ<Žv3cÛ@|"œT‰ð@]ŒzÍ%¸?²4<ó{b?©ýñõž?õŒSâÖ$@
ð%a¹X|¿±ùiã-¿â¢TˆîP«¿âX._ŽÛпâö²ydp¿ãâÔ}›6¿ç÷Àá‡AGNbll3FGL J0851.8+5531GB6 J0851+5528?ïú¦ãs ??kBþ#Ù?EdsÆ3ƒ¦??kBþ$?ïüŽÓߙ?QavŽLÝ?;‰a7eÇ?QavŽLÜü?ïïŽö"R¾?im
?`q	Ý­AÙ?im?ïíÃr[§i?L0y¹3Ôë?b<¤X–\?L0y¹3ÔÙ4FGL J0851.9-5229?åXÚÕÁÎÀ˜e"™‡üÀ9·üjIJÀ;~ðW‹@Ë`V{@ä¬{*C?À"'$17°?ª9Ò?ìÊ/ßÏ @	?âTžgà¿©÷؂ý9Á¿ªK̇,¯‹¿êòÇhýÖ¿Ûçœr<¿äÎý>.¹Ò¿ïÿ¹ß	eYAGNbcuPMN J0851-5228?ïê'!¼¼ý?gšTv —Ù?enÞCCé?gšTv —×?ïþöÓÕݨ?AŸ"Í0ù+? '¢%}ž?AŸ"Í0ùD?î¬ï8ÓÛÞ?›%-Žwr?¥1rÂB?›%-Žwp?ïá)¾ÁÜ?Z¨<RI[?nÖA>#ýs?Z¨<RIY4FGL J0852.2+2834¿¿ëGAŒå1@B×ÆÁ#À:]ÎpÀ<‹	%B¯¨@üܞ&H@'[··?ÆBèé­?ÂS7Q¥å?úåW¨]»@æèî–v$?ïÉ,«¿æì-_ߎ›¿å
ñáe¿äˆ—³æKú¿ð?ïê
_ÕR­AGNfsrqB2 0849+28?ïGë«eI-?™]Œ<ª°^?—Š"VÚ)?™]Œ<ª°^?ýÚ8G?£&6Lp£?‹™‰qí×?£&6Lp¢?ï¦ÃPYÇ?"A‹'Cá¿?œë'•ôÇ!?"A‹'Cá¿?îùŸ¥9²+?â0³Ê‡? f¬dÝ]?â0³Ê‡4FGL J0852.5-5755?Ú5
D<@oÀ!	3ã\[KÀ8j$咖pÀ;ÁŸr ¯@uƒ°Ï@J߈'4?¢àÏqì=?¹8Ñ,ØÑ@k"˜€"æ@r'M÷¯¤¿Ùg*±"r¿Ý÷"[nç¿ã·ž'6¦…¿ã¶°@O%'¿ç>Õ]•¿æ²\sž]NAGNbcu3FGL J0852.6-5756PMN J0852-5755?ïýRDÅ×5?/Ö¨K|?5mÙÑFY†?/Ö¨Kæ?ïømýÍUT?cðü±Ÿ¸"?NHʪ¯ ?cðü±Ÿ¸?ï¿´@(Á?ƒT@þ'«'?€þ/õÏ÷?ƒT@þ'«?ïÿ°ýM•D>úÒ>"š¬y?À¬š®Ý;>úÒ>"š«Q4FGL J0853.1-3657?h2Ð
+Ù@°hÀ9/²Ä
ªÀ;ӆžë2@ ­"Ýõ¿?þüÕ©`à?±upÅ?¯Ql^YR?ü˜.•>Á@ĖóL}¿æ­§"n>ø¿ÛžÔA
aX¿à
fÀÿ91¿Ú-'	'`¿â g߿݋c`wAGNbcu3FGL J0853.0-3654NVSS J085310-365820?ïÓm©e©?rí£2š¾?vIs+M+¼?rí£2šº?ïrè§]K?§Æ'ëb?'¢ë_Ö¶?§Æ'ëb?ïB>¬¡»!?'‰Î'U?—¸*kțé?'‰Î'S?î:C[Iý?–àŝ¤¡?®Œ[ÊK`;?–àŝ¤¢4FGL J0854.0+2753¿ìgÞ©31@Bóâ?$ØýÀ;þ—ó§,)À<öÀ
¢€@#kȂ»0ÿ¤¢F…‰A?ææPaAcx?ïþÿÝÑ@‹{ɤú@ûëLi»?ã&O?XZŠ¿ïÿßÿY'í?ïöü´>?Áâå¨eå7¿Ñ@Æcüÿš?Ô'»/ìVÖAGNbllSDSS J085410.16+275421.7?ïÛ¿˜ê­?lŠG6ì?rp 3Š©"?lŠG6ã?ïüxèG	?SAó7¥ü~??$8½ÇÁë?SAó7¥ü{?ï€iãiL?t7%¤c?å‡%¬Ü@?t7%¤i?ïû}V¢0æ?C§‡_ëŸE?B
¥w<fS?C§‡_ëŸG4FGL J0854.3+4408?çún_^*@D5~g,À:ÎKUhè!À<œ™ì¥°(@ô-.?÷Æ ÆI%
?Ŭ§¾J~?Ò¹]XJÅ@s]Å­ôš@Æm°Ãi¿ïþÞAê05?ïçè絆_?Òç¦læ³(¿Äbl†»ñ]¿çFm!ÁpοÖ5I£bQAGNbll3FGL J0854.2+4408B3 0850+443?ï}U:ñ¼ú?Ž¿ápb?UX¡È`Ç?Ž¿ápa?ïâBmö¶?'Mº÷í?m½'	rJ~?'Mº÷ê?ë>­Û$™w?®å"Ô÷R?ÃH"mš"?®å"Ô÷R?D‡u–?'Ä
‹Èq?¤Û·ˆ¦­?'Ä
‹Èq4FGL J0854.8+2006?ëqQR¡Š@AéÈ!laRÀ7'm¾iÀ;Y'àðp@@Öòj–!@>ü½U`…?"ÏÞF"0q?ª;·²@ºKÛ ¥'@£ñ
ݜ¿Äõ;Uìq¿àÍS‰Ò|¿ãá~ ›¿ãD_÷6ƒ¿æ²¥­Û¿â~25r
AGNBLL3FGL J0854.8+2006OJ 287?ïüâx:ÿÔ?4R—ûФ?8ì>(_&?4R—ûн?ïòÿ56K?tJ2ë³Ýþ?Z•"ñj—?tJ2ë³Ýþ?ïáÁϺä?r©ŽD!›m?n>æ0Eê?r©ŽD!›t?ïþfü½*?¼ÃÓúhZ?)—4-g}?¼ÃÓúgÝ4FGL J0855.4-0714¿êœeûCMz@7hëíúCþÀ:ÒdcVçmÀ<wÃیƒ1@ÑÑ¿¥ÇÐ@…ïbùÊ\?ÌhP ~Ж?Ø*´ÿ¦"Ó@	é{Y<²@!­ûü:N¿ÜÍ<žÁ̔¿Òþ=Áç¿ã¥Í"'± ¿ê9QZe§¿ïúÞ°ô?ïua Va¶AGNbcu3FGL J0855.2-0718PKS 0852-07?îÌXÜ¼h?£ða_bµ?£:w49i?£ða_bµ?î¯"÷°?¹Ä¥ë¢&C?¥Ð"öì?¹Ä¥ë¢&C?è[ÂÍ!?²œ_©›?͊ôËyÎ?²œ_©›?gý?"PrU?¤~"nù€@?"PrU4FGL J0855.9+7144¿çÁMmɆõ@AŸÄ~I±ûÀ:=ʝG¤À<H³B¸u@ñonwØ@§ú D®†?Éæ\Ukl`?Ÿ‹™·Ý¸"?Àe$w®@	"¤èWAÛ¿©…Ðäßh¿âõ°¡š¿èÃÜ-'àB¿ã¡Mø±W&¿ïÿÈ!ÂGŽ?ï÷A)@AGNfsrq3FGL J0855.4+7142GB6 J0856+7146?ïýY`}—?5¶À[¾ÔU?7U4üJ@?5¶À[¾Ôa?ïüã#á]|?^'ÿ±=Ù?8æàõ þ?^'ÿ±=é?ïÚ즖I…?uª>~ÙË?r‰¬´Û>?uª>~ÙÄ?ï÷{ÈÂ?D}ä]ÿh?Qn{Ïäå?D}ä]ÿ[4FGL J0856.4-5309¿Ì38bãIÿÀ3éBNY)À:™ÝLvÑÀ;õP~"Ñ@ "è[ôs@fq%Ý	[?Å%'Abu쿆:¾üpÔ?Ånø_»Q@ÇÔ/‰?éíÊsV8ò¿êѓ ÔÇ¿ç³ß@ñ¿åJZ«¼1¿É24/²u3¿ä3ÝbFF5AGNbcuPMN J0856-5312?ïä^ßy?g"AuÉ+è?kí¡ï ‡?g"AuÉ+í?ïþÄe¢Âý?E"þf¥0Ó?#¹¥ÓÐA²?E"þf¥0É?ï™xc§\f?†Íª7][Ñ?‰¡ç(æ`?†Íª7][Ï?ïéÛü³X¾?WM]âCB?f$L§BÒ?WM]âCG4FGL J0856.6-1105?ïÏÚp8÷K@5y*0U2aÀ8‡¶Šk(À;ôv_î@Ì/E½ÏY?ÿ.ÐG«<?¤r(çTã\?±y¾\òt@T©p¨	@
°4–	Â?æ^Å󔷳¿Øuaµ|¤¿àÙàvoÉ¿ß@dtß¿äÜ&$p¿âF•Ew–AGNbll3FGL J0856.7-1105PMN J0856-1105?ïüK½©?;'(ø{2å?=§j·¥'?;'(ø{2Í?ïÍ	Åî"{?"Øb¾0?y{¶B-?"Øb¾0?ïÀž³%£f?'¼DrÊÍ?°¦m.ML?'¼DrÊÎ?ïXe"O«'?|r¶ßE?"óMv
›>?|r¶ßE4FGL J0856.8+2056?ÏdÈõMÔ=@BD™÷LÀ9úÑáÃôÀ<<FipÜâ@7"/M>@'q›MÏ?º á!§¼?w(ø¿n?âÏbcøM@H[¦™Ý6¿ïÜô‰u?ìýçՒï¿âå‰\4´=¿â•€/eH¿ÝÝkëáe
¿â\&$pAGNbll3FGL J0856.5+2057TXS 0853+211?ïÐ_&0?wD|ÚS5?wÐtlçú€?wD|ÚS3?ïû,Âëâ?W†þú˜?COðôPxá?W†þú"?︷¬ ä?'±Âí§ªc?Òý÷ÆÔ?'±Âí§ªb?ﵶçû‰³?qtÓ·Œ	?''F'ø?qtÓ·Œ4FGL J0856.8+8559?Ø<£¢!@=(dŒq"À;c~h»«<À<¾¸‡›jT@·à™³Dæ@'ÉÜW"K?ÎÓw¾RŒ?À*ךOJ?î*Ö7¯™¶@Ň3:•¿ìøžï!‹?ãgc¼gú»?āBJR^¿çw5<滿àÆ7½¯l¿Ú¹9±ÊéAGNbcuNVSS J085740+860344?ïõtÍ;Ÿ!?Vـà€éä?UeˆÁ½*?Vـà€éî?ïþ\{Ÿš?Bý¹?*8F^4¿?Bý¸ø?ïÄ|ÍC^p?}OîµTþ/?}Á™^PÈV?}OîµTþ"?ïìL=G?PÉ冻T?cî³Â¸î‹?PÉ冻V4FGL J0857.7+0137?æ=]ĞŠG@<™;ʸÀ;8ž'7À<‹m{-È@…9C¬Å@tßÔŽ?Î.†¦!è2?Ëõ%Ü]Ž|?úPÞªDâˆ?ö¸Dý?ïðÓÊ¿Ç""FZ¿èˆóß`MH¿ÙeNëž¿ð?ïÿø¨ó©°AGNbllRX J0857.8+0135?ïŸ"u3}?`ÿÖ«Ñ?ˆ7b¹³ ¼?`ÿÖ«Ñ?ë<õ­?ÊCà=k¾¹?Ã)K—ïŒ?ÊCà=k¾¸?ì§&Kl«?¤²ü%š÷u?ºÆͤš§?¤²ü%š÷u?閭³g¬,?´)±\žNz?É¥I2aOO?´)±\žNz4FGL J0857.9-1949?ÖNʤŒé@0‡Ò"œ²SÀ9`ây|À<kc%iF@-_«·@'ãt®ÿ?¯©.Zêî?Ÿ¾E†®¹?죦-%Òø@6rÆÆù?ÖÙo]»¿ä¤øÝÌÏQ¿çH/^'\Ž¿åÐZ‹fÐï¿æ…bªð3¿ïÿ‹›ªAGNfsrq3FGL J0858.1-1951PKS 0855-19?ïük¢/lƒ?8XЫ]aó?<¢î"›Ü£?8XЫ]aØ?ïü.cgF?]s¼Ò`P ?>ŒäÇíÍ?]s¼Ò`P(?ïßJùg}<?oËË{qmC?pZƒLAbŸ?oËË{qm ?ïý.½A?%¹/õïg?7'¦ŠöK?%¹/õï¨4FGL J0858.1+1405?í¼Î=@A.j¨ëF5À:¾ã²Â_ŒÀ<oy¼"€@:ªÆg­ä@y\ã/å¡?ÆŲýî?½Ç;¾G"ÿ?ð"X6ù@±øÀƄ3?îÍÑ–0¿Ï­ò';׿è¥8hýœ¿è®½>¿â%Á?ÐÐh¿ïÿý¡UûŠAGNssrq3C 212?ïçtH2¾³?kOÆX2¡€?h‹·ÍAMð?kOÆX2¡€?ï±<<ìæ?'@F¥6ÁÄ?ƒ°ûðă?'@F¥6ÁÅ?îäȂ?–&¶@»*?¡¾_CwÞ¥?–&¶@»,?îًµ,0?ÿ˜P''?¢gF$­<ÿ?ÿ˜P''4FGL J0859.4+6218¿çpøiâJ`@CDhۋ¬qÀ:ÀõÄ<ÛSÀ<±‡O:J@4·jºÞä@WdU/?½åœQ"×ì¿}æñˆTC?½ðÆQ2¢•@u3`œ˜?ìžÊÆbO€¿Þ—u;Ê¿èú'`åóå¿×µ£euP¿ç§ÛACl¿Þð?ãÅ·°AGNbll3FGL J0859.1+62191RXS J085930.5+621737?ïùSIc`q?Dq09{K?J²Úr~:ò?Dq09{K5?ïýü
Í??Cäï)¢?0©—ÖC?Cäï)°?ïëv/ÛCo?l"ï‰ò?d‰Ð$¼'?l"ï‰ñö?ïø`ÔÄÑ?;:õÑö£?N̬ì¾?;:õÑöÖ4FGL J0859.4+8345¿îîxïôþ&@>MÊ:KUiÀ<êäåÈFÀ=5ôÆ/@"˗‹!†¸?ö¾0'}ó?Õª• Õ`?юcpàÓ?÷ÄÉÉMì@ž}"D¿ïÿðÇô ?ïùªæÈ÷U¿ïÿoì÷å?ïþ=BUºó¿Ñ¼§›dõοáñ@ÅÂíAGNbll1RXS J085916.5+834450?ï÷QN×Ô?P·®UzMà?Q]bQÐY!?P·®UzMá?ïüÏãÈ?QXÛáØ{?9€çñ¿û?QXÛáØ}?ïÁ'=?ˆzèC›ô?Œ¹›~pÁ?ˆzèC›õ?ï÷;Šœ}Ê?N¸"	Žíö?QˆêÇlC?N¸"	ŽíÚ4FGL J0900.6-7408?ïªÔžŒ{âÀ1úgèF¥×À:1Y³Ð|…À<7ä¼­šØ@~Ë?"@¢ùà0W?Şԁw
þ?ÉhÚÆ_ ?üö*ÿˆ
ü@	}Ð3´f?àbù"«ô¿ä~Áï#9¿ë¦°8Aí¿îg"¾Ái¿ÑAÿE¿ïü-""ÑAGNbcuAT20G J085959-741401?ïü·";i?EâÆÂ`Ç?:C^'Œ¶`?EâÆÂ`Ñ?ïûïÎx¶F?Wx"]jÃj?@@Æ&ãÖ?Wx"]jÃm?î¢oÀüoÓ?™ê´Â?¥Ùð9Ñ?™ê´Â?ïæÈà5"i?Zylٕªœ?i7Êk–:?Zylٕªž4FGL J0900.7-1243¿Ö&
œ>@5SÂCÜΣÀ:8èí"ÃqÀ<`ÎùͶØ@ßڃïŽ@"'A?ºh…¥pè?˜tŸ¡?ß"äRzv@VÞyzÐ?ïÿÞ§À£Ê¿Êši7Ñþe¿æÀŠt8¿â-%Òø_ù¿é-"BJ'k¿Ú&$"AGNbcuTXS 0858-125?ïûMçÖû?=À6²Ð
?C®È`¤°?=À6²Ð
=?ïþƒ̔û?Fv"õ]?'Î6°E	?Fv"õ\ú?'çIŸ?‡F$X/?‰F-—ú?‡F$X-?ïþÒtjn.?xïÝ0è?"عY(?xïÝ1×4FGL J0901.2+6742¿ÞžhØÕG@B‹kü¨\«À:iTK±¯:À<cۖ"+œ@¥À$Ä!@rü¬Žhä?Ã_5'n·y?Âf‡s|O?üvѵ(@ ov°?ïõ8ü Ïï¿âçí_>~ì¿çÃPýsˆ¹¿ä4ÂI¼´¿ïÿ¤€RuÄ?ä‰áàÛ!¤AGNbll3FGL J0900.0+6754TXS 0856+679?ïÙº×dš?ukx#(ýð?s""M²ò™?ukx#(ýî?ïß:mDù?ŽG(ZÁ%?pbÉt݃ ?ŽG(ZÁ"?ïµo¿¨@Ñ?'€+—H¤?'¤ïËÝ?'€+—H¦?ïW4sn€?'ÿ›<ò¶Û?•yq'0?'ÿ›<ò¶Ü4FGL J0901.4+4542?̊4e3xÒ@DªV"uÀ;É«¸€®À<ï[:¹9r@ù"D›?ü‹rX?á^$Ñq?ï÷ÝâsÓ@$ †å@í?³õ¿áën"cÔ¿ÁÞ/5L½ô?í_«–òm¿æwˆ,‰ËÆ¿ïÿԖũÃ?ç
ò¢IlAGNbllNVSS J090208+454433?ìÙðÑâ<Ø?¶é³Ï Öe?¹0ypîT?¶é³Ï Öe?ïÉ!ÃÓ?´‡G9'S?ÛDž¤?´‡G9'S?éûíI^Eå?¯Ã4¯ÊÄ?ÈJچèn?¯Ã4¯ÊÄ?êÞå݊ºx?´¿iaŠ¥Õ?Ąh‰Õ!?´¿iaŠ¥Õ4FGL J0901.5+6711¿ì~V[IòÁ@B¥Ÿ<pÊÀ;>Iç«À<Ÿ.X•@ 'è(ó¿*@´{'G–?ÂÝ`t#"¿…ùN'fn–?ÅúöÖ¶…Ž@æ"Ïíú?î'"2wL?Ö"D"™³¿äx7ÿ˧´¿àõ½ò>v]¿Õ¸"þ<[¿Øæþ§:l
AGNbcu1RXS J090140.8+671158?ïóp¾óG;?Sw¼dʲ­?Y'qÕ?Sw¼dʲ¸?ïüàx÷)•?\|eñK9ç?8ü8F³\œ?\|eñK9î?ïë -¹ ?jµá/ð•?d_ÒF~`t?jµá/ðŒ?ïáG×ßÀ@?^XaÉd?n¸( ?¿¼?^XaÉe4FGL J0902.4+6440?éÆæY³Öš@CàÁvWuÀ;A&"Ï:À<ÂFÊ¿¬S@ǯ½ó@)@ç*໗?Å°'åøý¿ OáGÎ?ÖùDåè¨@ïƃ°¿âëE=¡Ì¿ë'} <5¿Õ1e¾àÆ¿ã¸É_¯èæ¿Ü¬W¿ïü­/x"AGNbcuGB6 J0902+6444?ï÷hd\øX?LŠ"2/*?Q/7FOn?LŠ"2/(?ïþŒ•&{?G͜ëî¥O?.w6­˜YB?G͜ëî¥A?ïºÃl†œ?ƒÀ5"_?O$ÞY?ƒÀ5"_?ïø šÚ= ?<‰üÈ¥C?M}"—'ì?<‰üÈ¥Z4FGL J0902.4+2051?éUS'Áÿ@BàûC؜åÀ8ë+•°À<út¥ÄJ@𗏩*Ü@ã`dÄ¥·?§ŠI€¸³L? Ä©H¹,?ö;ßßÏ@hGn~Ð¿Ò<Àåä¿à5Úã1¿âIšHB‡¿âTä(3$ð¿àF4—·AJ¿éE‡=÷\mAGNbll3FGL J0902.4+2050NVSS J090226+205045?ïýd0?T¾?+éøJÔ?4Þ~Z
ð?+éøK,?ïýnàWL?F»†Ò»Ð?4ˆÿEŸ½?F»†Ò»Â?ïí 
=«?iµú Óã?b_òÂT÷á?iµú Ó×?ïü—‹,Ü?,R­BCÆ?;G¦™"?,R­BCÅ¢4FGL J0902.5-4801?»6í,‰L\¿îÃ"N®ºÀ9 ìt2À:ÞÿÕ8@›ýèx¤×@Q<\§¡?Îãî<Cñ?Üj¹œÄFk@Nªß<;?úi·¬T1[?íD8¿HB¿å¯m@u;¿çÐÓDM¸¿ìŽæbJ"
¿ïÓ±B'±v?Æ4Ü5JAGNbcuPMN J0903-4805?ÎDèȯߤ?Ì"¹Tґ?ènÅÍÔ?Ì"¹Tґ?ÐÛÍ;rK?ÓÛb¯Q*?çž2bFÚ?ÓÛb¯Q*?йËDtÞ?´Óaä‹8À?ç£}]Ő?´Óaä‹8¿?€c%Þµ¶?lӂ¾)I?ï¾s‡h…)?lӂ¾)I4FGL J0903.1+4652¿ï(tJ€Æ@DÉ}ke©¨À9ǽWäÃdÀ<{¬h©6Æ@òS™Z. @üc®%AÙ?¬¸9lÞ$¹¿¤€ýbäC?ö‹‹Ÿe@zêéz¿ÚÙaE?OK¿åÍ:°ÕöA¿ç0[b&eÅ¿åtáTù׿ÞFãÿ™RÍ¿ìàÁvWu2AGNfsrq3FGL J0903.1+4649S4 0859+47?ïúÐ4Ð?=ã·ï*ó´?D¿Ç,¿éý?=ã·ï*óŽ?ïû¢¤Æþ?U­>‰Yha?Auläóº?U­>‰Yh^?ïé§ÏÔ&?i¢<Q/B?fñX0+׍?i¢<Q/:?ïÖÂ,ʱQ?gÚ#Àç?tžéš§W"?gÚ#Àä4FGL J0904.0+2724¿æUÌ"b±æ@C÷Ä"`À:E®†¨YÀ<|Å<µ'ô@ïIp6t@~*Ã") ?Á—ø¯©¦W?ÆO¬e¤®?ÿ¿ôw5Áƒ@	¹H~?Æ]B Ç¿ç§"™2¿êß"²¿ê§}½›¢¿ïÿÞr¾"¿é´á¾ÌY
AGNbcuB2 0900+27?ïñ
	õ$N?^åX8?]ëì·cÀ?^åX7ù?ïìýø'G?µã¦8Ç?cmoº0?µã¦8Å?ïc"CýN,?‹!¦ÕPÅø?"w€V:`?‹!¦ÕPÅù?ïu¹ùG?|‰"Ì¿®5?'HÀ×½1?|‰"Ì¿®94FGL J0904.5-3513¿Æ̧Ý1@<Ù|ÞwðÀ9cЗ\¨À;Ô¯ÂÐʈ@'º.9¤<@¡&cAø?¹VÈ8¾b|?Ä@l³sà@#xà¼mÚ@.="‡¿Ì
#)$çk¿çw9ó@ÔÜ¿ãঋ(¿ë2O¨´¿¿ëÛÞ´UÞ?¤@ª; gAGNbcu3FGL J0904.8-3516NVSS J090442-351423?ïæÇV´c{?j¢–Oa?i8©KœƒÐ?j¢–Oa?ïùŸcg?cU<üÝ?I'rc"F?cU<üß?‡9<?›
c×"?§"çŒl?,?›
c×"?ïûD=Ë™?3Á^ü=«ð?BïÓ¥ž?3Á^ü=«ý4FGL J0904.6+4238¿íc3åŸ¼@Dø<÷TÀ:Ÿú D®†À<¨¦tsoc@tTc¯|Û@ôóg°?Ä©À˜¶ð˜?ÁǶb}#?úOSû)×?ùA˜‹Ò† ?í@֟^'¿åIÁêñ{¿âpŒû%¥¬¿â}5€V¿äpŽ•·¿ïÿï¿@PAGNfsrq3FGL J0904.3+42404C +42.28?ï¼iµE÷?:¨_MÂB?€å'® f?:¨_MÂ@?î돛z?¯^š·¤H·?¡N÷öHx?¯^š·¤H¶?ï›0qx«Ô?ƒçF.Yn'?‰3ã¡Õ
÷?ƒçF.Yn"?éÍYÐK<?¬;çµÊ]Õ?Èʛ¼¾Ó?¬;çµÊ]Õ4FGL J0904.9-5734?î'²¨–©)À$«>݋aÀ7ÉÜ_çÇ$À;IŠ]ÜT@©b"@Úºp©¶?˜#yç;?¥´t€b0@
6lmçd(@"›æ¥ç¿xÇ!€òól¿â$Ÿä6v¿äFÿ=T<¿ãw÷*|«¿ælŒñ«¿áÛ~ AiAGNbcu3FGL J0904.8-5734PKS 0903-57?ïý"݉Ë-?-¨ iOáÊ?3Y±¦•
?-¨ iOâ?ïú÷ç›o\?`p4'D$?D a'B‹?`p4'D+?ï"ì™?~þm­ß}?~¶	³|ýá?~þm­ß?ïÿĕÚ}Å>ö0cÚp½u>ýµÁÞµ>ö0cÚp½~4FGL J0905.6+1358?ÆÓà¾Þf@AûÚ¾'œÀ9PvÄ À;Ì(Hôe˜@:grÕàr?ùv÷xr¥?²‡›À:m9?Àk.¢)àú@ll—ØÏ:@
õÁòSD ¿Ú½'Æf>¿º{Ýñã1¾¿Óžœ"_ü?¿Ñƒ%Nn"¿àäëa¸VÉ¿ànÀY!AGNbll3FGL J0905.5+1358MG1 J090534+1358?ïÔöŽ½Û?¤NG˜—²l?u"¸þ¡?¤NG˜—²l?ïò󧰊â?lçílL†?Z°žê;?lçílL‹?﵀[Bd?…§»=KtI?'Ÿé/¦Ä?…§»=KtK?ïk‡»J$?tt\iO"?'Ÿ6»ž?tt\iO"4FGL J0906.2-1707?îïTØÈ@3¾G'ܾÀ;"æ>ÚÀ<l»êý9@ x–†>Èé?þ0M:Ev,?ÑÕn'€ñ?È;™¼)<?øääÖ®ÍÞ@4ô‰)^ô?ïÅì=«\:?̵FÞ¶¯)¿£O.D³Å¿Ú>Ù#ó$O¿àœ¨AÓ	'¿ïòË.g˜AGNbcuCRATES J0906-1706?ïò€,ä$ò?_:G…Fï?Zÿ¦7¶I?_:G…Fá?ï©XvÇã?¦|É@#Œ!?…©âN9Fã?¦|É@#Œ!?ïkæã•?…•Ôù.¿‡?‹åX‡ð?…•Ôù.¿†?îMu4þvÚ?"³ÌÓÅî?«(¬°'O?"³ÌÓÅí4FGL J0906.3-0905?í'J^5¨«@8'sÕº²À9óÿò"³À<Qäþú2@]oqÒÖ@^쿱[W?¹*³Éƈ?´sßrkØ?ûåCÃC@‡-ã"ã?ï;ái\æ?¦½nú£¿ÝÞa_@'Q¿âØ)Âq)8¿ç!½T‰Å¿áŽýÉÄڐAGNbll3FGL J0906.3-0906PMN J0906-0905?ïüä\¹5?3™(»·¾?8ÝÂ6cz?3™(»·¾?ïý&¨«
u?ITA¿ÄÀ¯?6ʺ§¬h8?ITA¿ÄÀ±?ïÏ%ã6®é?{ÿ˜5?xmd¨Š·?{ÿ˜@?ïú'´ŽÀ?5W«U6³?E¹-Åù?5W«U6Š4FGL J0906.7+4950?èíTp"@Dõn?x»ÔÀ;•X'ßBÀ<ÚpΟ4ä@JÏß%ë@RÈqz?Ì\K‹*¿Kñßő´?ÐØV"¡jž@*6jX‹?ïýùà¬'¼?ÈÅq¤2#ê¿ìâ?z¿¿®UÙa–Ú¿é×»]Ž¦v¿ïåj‰
ÖAGNfsrq87GB 090322.8+500444?ïøn"1&|?VõüåYȪ?NE³;f"?VõüåYÈ¡?ïýjH•F?T˜¢€ˆ5?4­¿#UÑþ?T˜¢€ˆ(?ïŠ(Îî?•|ÕÖ$áÜ?œŽºæ"?Á?•|ÕÖ$áÜ?ï÷×é¹[?Bô¿§90?PQî,LÑ?Bô¿§9V4FGL J0908.9+2311¿ïf©E¢@Cô$_ZÙjÀ9ܺã–<îÀ<%˜°eù@ çW˜BV'?û
RH¢0A?¼Âs,lã?»óÈd2Z@M€ÿnàˆ@[,þåÑ?ïÀ¦]ø-Ï¿ãIJh!R¿áŒ…0aÈ¿Ôð¤ÃCa¿Î-)ÙÃ*b¿ãö9þ(kAGNbll3FGL J0909.0+2310RX J0908.9+2311?ïýPÒ"Ûä?/Nʘ ?5yné æ×?/Nʘæ?ïúëšÈÔõ?XV*ý
¯	?DQ"ܬ*Ú?XV*ý
¯	?ïîmÚsJì?hµàoÊH?a'%Œµ_?hµàoÊH?ï¦wv=ãØ?r¥ûævû;?†b"p‡	Ø?r¥ûævû<4FGL J0909.1+0121¿í©.·Øh½@>í/IŒ;À8SÓíçÐÀ;¥­'ž"•@Á˜€iò¸@ì´^@ý÷?žT©œéQµ?¹_¿p@
¿ó v@ð8æP?î‹#Ÿ—_ƒ¿ã¯Þø¿è>þ#†î¿å¼Ù¿úVs¿êìÔÿ÷«¿ïù0¾
í)AGNfsrq3FGL J0909.1+0121PKS 0906+01?ïøò1ê]E?H
`dxâ
?L78VŠéê?H
`dxâ?ï÷8>ÿd?n2~…u$Ò?Qã':°?n2~…u$Ô?ï#ݟãA}?"qv¡¼Ö<?›"L—Ðv?"qv¡¼Ö@?ïùmÿé¹?<'$þÎí
?JK"Y?<'$þÎí4FGL J0909.6+0159¿â·Š(JÖ£@?\œÃŤÀ9DkHMwÀ;ëÛd?D¹@"ØБ(@ZÜ
²p?·` SÇþ?¿äq.@…@Õ"Ü£Ú@e骩}¿ë"ÎÁnŸÆ¿ÜQj€ÒMj¿ß;t€¿àW1	G|¿çDP'èË¿èx¼_eóAGNbll3FGL J0909.6+0157PKS 0907+022?ïÒ¬VÛ{<?zO,±°a'?v©Ô'Baæ?zO,±°a%?ïµA-Ú÷Ó?¥1ì›a57?'¯´‰B
Ï?¥1ì›a58?ïŸJ¶m™}?ˆµÄï`?ˆ-Rd™¡
?ˆµÄïd?í­êiÕTA?šæ dÇ,?²¬±U]ñ?šæ dÇ+4FGL J0909.7-0230?îŠå°œÀ@<þrÚ/­À8'æ:\aÀ;ƽÀÀO@#êç¿í@@Ñå:Ü?£+w'(ãÏ?¹ºÙ…AóÀ@mmÁ¤{@K¸»÷¿ÁæƒA¾fX¿ÞOX,翗¿äÆÄ	¯¬+¿ãò<'Î{¿ëùÍNY¿Ù#''%ÎAGNfsrq3FGL J0909.8-0229PKS 0907-023?ïõãýÛU?OBÂ
÷7•?T8IUØÐ?OBÂ
÷7?ïëàÇc?€¢ú'>×?d8ùœø8?€¢ú'>×?ï¦H^E¶?—älŠ`]æ?ŸK6ô7Hù?—älŠ`]ç?ïÆO"èáõ?hGÃëmQy?|Ø5‹?hGÃëmQu4FGL J0909.7+3104?ìU¯O'c@DõË£!hÀ;PKúˆÈÀ<ÎañŒŸ¶@ 7‡bàJ?ýñk—þŽç?Ë£ƒè­S
?·ÑêK¸»?ì[›Â=Ҟ?ýž…´Š`Â?åÇà~ÛRL¿Ñ›Dß­úû?ÊÛÿ…0Öâ¿àxzЀ¶t¿é6añŒŸ¶?Ä]Ý@bp¸AGNbllB2 0906+31?ïò×&¥¤"?S!Ú-]?ZQ²´¶Ö=?S!Ú-]?ïõ½7bÍG?qwG‡Hž8?T…':erú?qwG‡Hž9?ï`g¹ƒ"@?xû™'&a?"óϛ¸?xû™'&d?ï<¼>Ua´?"òM‡?˜hx5SÉ^?"òM‡4FGL J0910.6+3329¿ëËÕEÈÖ@E;\B 6À8܈'=À;ØÆï=:@¨Xx4?þn­È$Ç`?ªˆ͝‹?§yê&Ï͈@ì6Kìh@,ñê­Ø?ïõ@YŠ?Œ²QUø¿áS£ìó¿Ù
µà¢Á¿âêÑÀ&¡*¿Üj5"_õAGNbll3FGL J0910.5+3329Ton 1015?ïú¨Sæˆ?A
«7€ G?E^°eßßÔ?A
«7€ X?ïÔK¼?"/»7Jå?uúZ!ô@?"/»7Jä?ïÎÆLËV¾?~«2Å\Sy?xœÙšT X?~«2Å\S|?îH·­Þ…M?–½.ØËS?«t…"«+?–½.ØËS4FGL J0910.6+2247¿åWj"¡èï@D;`(^ÄÀ:È­ƒ[jÀ<£_ëøâ@Fá'+¼@Œ—£TY?·à…;h¶Î?ÅlÉKR@/–@HÅl@ÜD!×?ÁâIá n¿Ñõª§&¿ãTגùlh¿ã·#240¿î0(QWáh¿ï骝i2AGNfsrq3FGL J0910.9+2248TXS 0907+230?ï©6¯‹æÌ?€Ø'bûZÔ?…²TM&?€Ø'bûZÕ?ïú'h«öÇ?fŠ	§ð$v?Eº]P$ç8?fŠ	§ð${?íU­Rîlþ?£Ç«ˆ8?µR•hŒ˜?£Ç«ˆ7?ïü1xZ•?.'ÉEyn??~t=+gv?.'ÉEyn04FGL J0910.8+3859?À¡Hm]R@EáŸÂ¨‡À:Céœç+ôÀ<‰>xá"-@1o¦Öîå?þ#êÛ«Œá?½R'KÕÁ?º<kÁ:d?ÿ	9d¥œ@
PÌG@Ü>?ïµ{™>¿à6]õ~œ¾¿ázd ¯…¿Ó>.#~à0¿æegʵ¿åšQ_™¿AGNbll3FGL J0910.7+3858FBQS J091052.0+390202?ïþÉe4­?¡øºÁ…?#i®œµE?¡øºÁÿ?ïý;˜îV©?K¶·Z8L?6#8J­?K¶·Z8K?ïõ¶àçN?bµEG÷?T'>1cÚ»?bµEH?ïï]53 ?H ±yM@¯?`å¢ÊÌߜ?H ±yM@Î4FGL J0911.0-5047?¯'Lvr«¿üð¾'dÀ9v,:ñm–À:åÉêpL@F\…¼íÝ@Œã›EkD?ÃÄxÖ*š?¥
$:qì?æìË:%•¼@s]Å­õ?îoÚê¿äÍ]"̃¿êL!@Âgï¿æ÷ ÈÍcÌ¿ÞMŸ½~ü¿ïÿâ¾÷!AGNbcu2FGL J0910.4-5050AT20G J091058-504807?ïèƒñï²/?o^p©mµ?g|MÐ~?o^p©m¶?ïýsQ(‡Ñ?XÏ\')?4ev»Áy´?XÏ\'?î!Æa2?¢ÏP±†Sû?­ãŸîéìÊ?¢ÏP±†Sú?ïãï5Þl?]]f_7?lpÊ!"Ž?]]f_74FGL J0911.7+3349¿ã…x;ÀOx@E_0"'À:}7褚À<FÞ˜¯@1{™>@…¼‡Û+4?¿Žù£?ˆ™õ'œWî?ˏà³3ž"@Gò[§›?ÅïšØL¿é,*?ï"2¿ã®"&±¿ãhpa'ëO¿áRG•ÀÇ¿è‹Å .AGNbll3FGL J0911.8+3351MG2 J091151+3349?ïߜš?dA%ђ ?p1²ó¸}Æ?dA%ђ ?ïýôXÚ'?R8Í=9åà?7ø]9.ã?R8Í=9åÝ?ïåõ+EÀµ?pÅ*#=JÃ?j
Ôº?JÆ?pÅ*#=JÀ?ïÓ3šâŸb?a¨Cäÿ™?vf2Ž°NÖ?a¨Cäÿ•4FGL J0912.2+4127¿ÕÇö…7Äï@E«ž¾œˆaÀ9ÍÆÇÐÀ<cJw—@¼³äsˆ@\±×?®žsóí£?¦-4@¤_ñ?ñäB"ßÎ1@€"[ï¿ì¿ÚÆÁ—"\¿âµŸSí½Þ¿èܦÿ³©æ¿ãµZTà,%¿â븮㮿ïÿAÿ~ÐÀAGNfsrq3FGL J0912.2+4126B3 0908+416B?ïþ×ÿÎ?#¥Q5ˆ™…?'†	ß?#¥Q5ˆ™?ïý1=#­ä?M""Âh#a?6vâìÞ?M""Âh#Q?ïêsrË?gªßËFÚ?eŒè4ù?gªßËFÚ?ïÿð"×(>Ö»Du½>ÞÖQ¯Òr÷>Ö»D€¹4FGL J0912.2-2751¿íÝ:iz0É@+×ß°Õ À:w©"ÉÀ<´9Xb@(½Ã@Ë—¦zS?ź†c±Ö&?ÓZ]-W§@
"Á{_ò¯?ýæϧóyŠ¿£ÝëœàdÉ¿Ý»÷<Œù"¿è_}¾ò™¿êL'ÅA¾¿æʳ¸(ÐÚ¿ïüƒ]œ"AGNbcu3FGL J0912.6-2757PMN J0912-2752?Öê£×ñâï?̛/œ¡j·?䊮‰?̛/œ¡j·?Ðÿ¿Þ†Ÿ?Ïrz´`)%?çø€ ¼±?Ïrz´`)%?Ýüp†ë+Î?½5M0i­V?áǼŠj?½5M0i­V?Ìíc"Px?²}Î^aÏ(?èþ§ëâ?²}Î^aÏ(4FGL J0912.2+2800¿ë0ƒï¥}¢@Dìä¸{ÜðÀ;REå"TÀ<¸é_ªŠƒ@!þfUõU¿µt'ÞÛ?æ$ãåF?ïÿÿÊPË@Dʄóð'@Ô«-•º¿ïýH_ë""?ïÿå"m/®¿ébP¢Yܕ¿álpk¢æ?âKYÎy¿åÍ+Í
dmAGNbll3FGL J0912.4+2800RX J0912.2+2759?ïÊ=5'À?¯WU؂?záe>û ¥?¯WU؂?ïü©1òâ?V1wø-&?:¶po íÀ?V1wø-?îÜtsX(^?•KÇd]?¢8¸Ê}z'?•KÇd]?ïü£¥î @?AÜùB=¶?:âЎý÷¥?AÜùB=¨4FGL J0912.5+1556?ï÷šìÍr@C#,¾¤ëÝÀ:™&dî—"À<uÄsa÷@!%³fm?ý§8ô=T?·—•á|Ý¿«¢%¯<4?ó$ہ›v@½íc›/ò?âúw_²íþ¿èSľ
'*¿Ó˜Í¡ˆü=¿ÝPô¤­¿èæló"
?àã"C÷¦•AGNbll3FGL J0912.7+1556RX J0912.5+1555?ïú•È(|6?E3z•1,y?E¨ß^.‰?E3z•1,"?ïûýñuÔÁ?R»YÞ½?@:(¬øü?R»YÞÇ?ïʞ˂ê®?ªW~ÃèÀ?z°š>Š¨X?ªW~ÃèÃ?ïÂÓ8ý!m?pF)KäÁ?~–coIè?pF)KäÁ4FGL J0912.9-2102¿È;…{«d@2|!ïAÀ9.qÊG·OÀ;à{.t‡'@ @É1aÌÏ?ý‹ÞÅó"¸?­ÐÂ¥¬wm?ŽÈfƒ4C?ဦÿÝo@Ÿ°É6¿ÜÛ@­ð¿åŠÉ>$(¿Ùeåvø…¿Ü=Ì4!¿âø?Â7È¿¹U@Ï(AGNbll3FGL J0912.9-2104MRC 0910-208?ïø®ï ›?LŽ‡«vä?OíDC}–?LŽ‡«vÒ?ïüq3?W(͸çxp?;÷<w^po?W(͸çxl?ïâ	±Ô¶ó?t}–<¦{?möN+I¾?t}–<¦z?ïÛ›_S\?b"ÜEÉ?rv2PVQq?b"ÜEÉ4FGL J0913.3+8133?âíçøß@?ʝ@îÙÀ;qøòŅÀ<öŽhãï(@!¿ì÷åK?÷ìˆÚ.µ?Íßa$FE?ÅgY«m´?ûB=ú	F@Sx]3â±?ìäâ½ÏÙÈ?ì6«Ô.Á¿ÚÙ=—À|¿Úͬ;ç%?µ‡Kä/¿ÒÀ>ÉêDAGNbll1RXS J091324.6+813318?ïùkHåþ—?N}Ëüˆ?JRÜh¥Ñ?N}Ëü˜?ïýG¿U?O9WB ?5ǂÍc?O9WB ?ïÅôNÃrw?‹3ïÿàl?}؞FÅ@?‹3ïÿàq?ïõ¤HGòÿ?IPŸŽÓã?T·opC?IPŸŽÓæ4FGL J0914.1-0202?êÃD]À@>-inX£/À:è½±¦×À<[íâÇ
@Á_»ýF½@ûÜA´Ö6?Ã&¥]Œù¿§I#4{S?ä!7Ì¿a?þØ^€¾×A?ïù%P¡F¿ÙsûD¯\y¿ç™$(Ô4 ¿èyÚçÜs¿¤L߁°CÕ¿ïlìýļ]AGNbcu1RXS J091407.9-015949?ïë\ŠDL™?ae¿™Z*?d£u»³f½?ae¿™Z+?ïö2>;"ª?p2f?S›ƒ‰º«ò?p2f?ïp†oô?‰Œ÷¸ï}?'ïÏ2n?‰Œ÷¸ïz?ï¸
8~À?sYXxXfõ?ý|qàO˜?sYXxXfó4FGL J0914.4+0249¿Þ4¼šóüÚ@@h&Üã›EÀ:æ*|«LJÀ<X˜џš@¦A¡µòÁ@Ìî?äž?Á!95«³x¿°ŸíË{?ðn"ü¡¦®@Ӈ[Ôg ?íòãâ"¿é.î•tpë¿êt»(_šš¿âMaa™Î¿×&IaÉ¿áÏïH²AGNfsrqPKS 0912+029?ïòüü§Nþ?\@fpån?Z±b
?\@fpån™?ïý¹¢÷?KÁüA#òT?22èCîI?KÁüA#òL?ïÒÇCQ­?y÷Y~&bŠ?vœ^~×)E?y÷Y~&b?ïñ9"ì?Kh}ìrB?]ŒØý*[?Kh}ìr@4FGL J0914.8+5846?ï¿Ræö§@D§t¼j~úÀ;U^½ûx²À<ö›]¾÷ø@b#¨§?úåP׈èq?ÒÜù€4à?ÑÃa~ ?ÿҖÀ¡E`@':g?ï¢w÷ˆ¿Ø÷£ei}¿á"i·S¾Ä¿Úa'¼]hç¿ÞÁ[)œ\¿ïÿíöé	AGNbll3FGL J0915.0+5844SDSS J091451.54+584438.1?ïý —'ü?F4æI½?6ûCè ?F4æI½ö?ïúh+þ?YîVCqîä?F_S ì"?YîVCqîæ?ï{­Ê²ß?Šrdbêë?ŠF¼É¤6?Šrdbêß?ïœÿ¦—?r'àz¯šw?ˆÿ|ÀZ?r'àz¯šz4FGL J0915.4-3027?î›éÊ<V@)g¢xåÅÀ9ÿϾï"xÀ<49O¬æ}@
¾ýVW{@º–ic?¿Èûà3÷?ÄŸ€
s@Ûc[+J@ª¾MØü¿à–/¢!M¿ÌqÇXÅʿ㚾È'Kž¿á™!¶3-¿çY$Hµ¿ïýü_Œ'…AGNbcuPMN J0915-3030?ïã4_
½c?eÆúàÎ-?lË òBœq?eÆúàÎ-?ïݘŀŽ¤?…뎮u€?q3?¸­´?…뎮u?ïR¥ÜÊÌ?)C:©d?•«Df¦|Þ?)C:©d?ï["ƒ5¨c?|·:Ù¨•µ?"™Jów?|·:Ù¨•¸4FGL J0915.9+2933¿Óxõ‰ÇþØ@Ey…H©¼ýÀ8¥	pÂ
À;-M@$³@áòNço?üN™´?¥à¿Ôu?´FƒÇö#]@#¿µ'@	kèhߒw¿Û·‰lü¿×üè]÷×è¿ÚnYåN£Ò¿Ù‡'›x–ë¿âcÆ®¥šY¿á—ÙÛ©¢AGNbll3FGL J0915.8+2933Ton 0396?ïòHeæ?]T€â»È?[óoç44?]T€â»È#?ïÎxQw±Q?'ptp?xÃ×D'X
?'ptp?ïqx­ç-¾?'ä&f\|?'ÐêCHC?'ä&f\{?î=P½GUv?ˆ…×d
£?¬*ô+Š¨£?ˆ…×d
¤4FGL J0916.7+3856¿rõpül6@FؤTÞÀ9ÇÑq6À<Z«m×sð@}Š6OGf@ ôQvY?¶<Œß].k?»éß,Já¦@#³é¦ø'@ş\§ê?ïøª*s¿áŠ2¾™-c¿åV«¾	e"¿çøä¸{Üð¿èÛނ׶5¿Þú@MxAGNfsrq3FGL J0916.3+38574C +38.28?ïùE¥Ö-´?lyzlÈ?Jéh§I.ë?lyzlÈ?ïü…¶ß˜?TuÜ|[ †??ÛÒI<A?TuÜ|[ x?ïÈbãÍn?wFðZ^ì?{ÎôŽHæ?wFðZ^ó?ïë$"Ǭ?P§7òËÀ?dÛé{8SÎ?P§7òËÊ4FGL J0916.7+5238?¢Ýy¢‰¼×@EƒÖ¶Zš€À;96À<éaB:73@ ©³"Q]ì?ûbU)þK?ÈvnfÔ?Àž«;ØsI?ùŠý¤/ö@›‰¿ÜÏN¿â±/bn4;?ï[$éÄT?¶œ µÍ¢¿ÝåœFó¿Ú/¼TS¿è®ÏÁsÓ6AGNbllRX J0916.8+5238?ïî6iàw	?bÂ̞QH?aɖˆöÈ?bÂ̞QK?ïüH†A?XÛCqXüÔ??ïÍ»Íø?XÛCqXüÓ?ïÇleô"ž?€­†ñöžm?|IÍî°Ú?€­†ñöžk?)­¢?qÀ¤Üiª?‡õ"—Y?qÀ¤Üi§4FGL J0917.1-2131?èoè+ª5Y@2ëÊÙ­…àÀ:¿ÒóW{À<WMÒ@ê{áLá…@ÊA¤åþ?Àoºx¿ºc%¿,P@?üuuGª¹}@@Ÿ¼}¿ï»…|¬#	?ëÈóĈZ­¿åfl{S]u¿æ¼QքܿÕsϛY–¿á‹½m´8AGNfsrqPKS 0915-213?ïçÆFK*¨?~Úûlå+?h9¹´ÕWÕ?~Úûlå(?nPwœ?¢«Z瀙?€œkâ>¥?¢«Z瀚?îf¯x8(ï?¡î¼×Ý;?©•|}q ?¡î¼×Ý;?ïãØ29¿?`üÅö×Ôl?l~'ÍÆ?Ô?`üÅö×Ôq4FGL J0917.3-0342¿ì»"mޗ"@=æ»frû À;.Ɗ"lYÀ<˜-שŸ¡@!ºÏ ;Ê1?ü»-Çüƒ?Æ˛ÊKh3¿•ò†Hõ?Ñ%'×µ^?ÿCûàa¿ïûjÚim'?îƒÓ"g*²¿×Êühñ¿â×ßð•ÿ±¿Î-›™¤{¿Ô￀ˆühAGNbll3FGL J0917.3-0344NVSS J091714-034315?ïüU ìA‹?@ÑÛ1îT?=Vøó©²?@ÑÛ1î[?ïý8™~¸ò?Oh$þU?6;4
8qB?Oh$þU?ï⊌¢?oÐzÖµãª?mèués^?oÐzÖµãŽ?ïÓqýûÁõ?i­'¶¼-×?vGÞ?i­'¶¼-Ó4FGL J0918.9-0625?æ|'­P¶&@<©ÏF#ÐÀÀ;(ZµX<À<§ƒ]2L@ÅÐon¢Ë@Êô¯ú?ÏâXûå?Ó'{ˆŒ?ûûCµBm@ó^'í/Ä?ïã¯1±Rô¿Òþ"Õ½6W¿âòžM]€å¿èú'7¥ˆ»¿ÜõÿRÛð¿ã¢"Ÿg8ôAGNbcuPMN J0918-0628?į̈ånrÛ?|DB?ì»õ?y«HƑâ?|DB?ì»÷?ïø|À°@?a²¸Õëj?Ný>?a²¸Õël?îN7'Ï?¡y…ÃíÝ?¯ì‡Òû?¡y…ÃíÛ?ï]	Ú³?€ÏiJ?"^Ü$©œ1?€ÏiL4FGL J0919.3-2202?ïæpNâ+!@2ù€ä–íîÀ;rûbÓÀ<²'{J@!VhÏÍ2M?û‡"7Üæ?Ô"D¾Â?ÂÊ·H×	g?íds²C­@Á5±]†?ëޖxÓ¿ïynìFå˜?à»ÙÊâ¿å5ü;Oa¿Âák)¿é$ô^NAGNbcu3FGL J0919.5-22001RXS J091926.5-220052?ïü¢~(®?<÷…%¡õ?:ïº'Ö?<÷…%¡4?ïû'ß!t?]äՎ•-L?AôƒŸz4z?]äՎ•-D?ïÈ9"ÍD
?~`S5"?{ãn™]û(?~`S5?ïìVs''L?Yï09 ?c©Œ}}³Y?Yï094FGL J0920.3-0443¿àº…x'3@=ñ|^ö/À;+×õûÀ<W$ü8Ë#@˜"vm@wŸ©~+?Ë\(	‰k¤?´€ÊjÇÊ?äIRÄÈòM@	 ]Ötì?ïòãízÂ>¿èHyìU(Q¿èjd!舿ê1HKÿ¿á½¼>	P¿ïùœÙ¿úVAGNbcuTXS 0917-044?ïÿŒgÇÒ?'k‰ÝE?æ{"À?'k‰ÞŒ?ïþf 8	?LdZoWhˆ?)Ÿ•üˆA?LdZoWh¨?ïÝ}úë+"?t¸Ñ4NCû?qAŠj6ë?t¸Ñ4NCû?ïóžŽ&cï?Fÿº
ø+?XÂã³8$¿?Fÿº
ø*4FGL J0920.9+4441?ï*Åêý³@Fgb(EÀ7ÉÑæèÀ;8àò¿@Ì8¢2ðB@#szK¹? Í&Ü/7È?Ár3y)6°@&…ô¡'-@®uµŽÂ¦¿œæAE£*ð¿Þ%[Z™ª¿å&=·³à¿æ°üÂ]޿ꨢ ÿ>¿íêi*fAGNfsrq3FGL J0920.9+4442S4 0917+44?ï+eðz)Ë?—mbÛ'8?š"AðºÆ¹?—mbÛ'8?ïÝꆤò?'—¡=•%m?q
¼­ü‡g?'—¡=•%l?í½'X'Jq?¥4ɨ+J?²í;m¬n?¥4ɨ+L?ïQ/Øhœ?"1!ŽÙÅ6?•Údòì?"1!ŽÙÅ84FGL J0920.9-2256?à(:­É—Ò@2¥…7âÅ]À:ÙjÿR[À<€[wõÚã@!$ï$©Á?öâñLO?Ն¥ 5"?Ö¬ƒP?ÿýf¤S1?÷°o̖œ¿æx="ßEu¿àNÏÜKÅÑ¿ÎK*
j'¿»Õ9'ØŒô¿àš¥½ê0á¿àõ–AGNbll3FGL J0921.0-2258NVSS J092057-225721?ïê]~¸BW?e>+ßuJ?e¢G½©³?e>+ßuP?ï¯áÿ¦¼Š?íæ¬Æ4L?"€PÝ¿?íæ¬Æ4K?ï`´{`Û?%'"ßÚ/?"ép"䜀?%'"ßÚ/?î6ä°I>?"£Ã‡/Ž?¬'´ûo¼?"£Ã‡/4FGL J0921.6+6216?Ƽt£C¼@Dᆘ5À8LPíX^À;ê"lXî¯@"ýð[GN@ÇìoíÏ?œMÜ#N[$?µFß•d¬@2è8ªk@¾j£Œâ|¿ÆÉ™;¥È¿áΪó^1¿ãÝ_~Ù¿å‹V	÷Ї¿èém¢ð¿ì,ÉVö†ÚAGNfsrq3FGL J0921.8+6215OK 630?ïëԍÐý<?"â9vµ/?d+r/ÃÑ?"â9vµ.?ïñW÷Àï‰?wR%ÄÇ?]P~ îC?wR%ÄÅ?ïÊnñ}m?}ŽÎà¡?zȇAIô?}ŽÎà¨?ïÿ¤3åQÀ>ýAó¬_?ó«ÆO>ýAó¬^…4FGL J0921.7+2336¿ææŸÌ'@ElÍJ¡À:<—FÙeÀ<xÀŽÐè»@¶õ¼/E¾@y@þÍÐÙ?»Ø5õ…S?`¢1Áä©r@K®+÷Տ¿ã­ÕÀ­¿æÝݖH¬A¿àîŸéiæ¿Ú$;ɄĿéÔÞF-⿸«äIìPAGNbll2FGL J0921.9+2335NVSS J092145+233548?ïû<dµ2??¡oÛ×ø?Cm+7Ÿj??¡oÛ×½?ïþÌÆ)?GWèkË?.c3ž
}Ü?GWèk·?ïζ•iō?~´»ÕÄ(*?x¤µK9¬?~´»ÕÄ($?ïúC9—–û?6Àÿ¾HŸ?Fó¡¤?6Àÿ¾HŸ
4FGL J0922.4-0528?Þ%j'@=푼U†DÀ9õ×CHT-À<WBXj$a@í™IÁÉ@[A9†3‹?º½ó×þ"?Áû¿i!@¿l\I¬ò@I1!`"?ïú=³¿µ?±'Ò*.Ò¦¿á7€—9î¿äW~Áüå¿Þ:Ó²¿êc'@ßÄ AGNfsrq3FGL J0922.4-0529TXS 0919-052?îÏËÅ-Íù?¢Áóñ•ŸP?£C­# c?¢Áóñ•ŸP?ïtH¡Ã™À?®ˆâÿb³?'vënjÇç?®ˆâÿb³?î\ÕüàÄ?žñïì9
?ª?' 1óÄ?žñïì9
?ì¤^C¶&´?œá²	1Î?ºÝ
âNÊa?œá²	1Î4FGL J0922.6+4454?ëDGo'@F‹«ud0+À9»ˆpSOÀ;;èné§@lY­ñ?s@µyyh¡ª?µºÎaf;7¿·B~"%¥@¨š¾\ǁ@zxnљæ¿âEà_PÈ¿ëÕ®Þ]¿æ4ò»sÞõ¿ã'
?ىʿïò5ýgõ2?îÈïÈzWµAGNbcuNVSS J092235+445749?ïöF«w?`J†ËÁm?Sçr©×¹?`J†ËÁu?ïïçM/í?‡Œø2"½ï?`à²ÐÃ?‡Œø2"½î?îõlÂîÎX?"[ô£¾Ç? ©3Ñn?"[ô£¾È?ïÞGhöw²?f'ù–»¿?pÜK"Ä's?f'ù–»»4FGL J0922.6+0434?±~_Xº@A»´_½ŒÀ9Òþ?5 À<7•óëï@šÙlmf‹@͉ößÆ?°&Ëƽi-? 	ߧÅ×:?ëG©Â†¢Ç@=zœ©C†¿ 'Ѐ>T¿ßz}	@¢¿ç.,Ε#é¿èëaŠR¿ç»š?±Æ·¿ÖŽƒ»áÂþAGNbcu2FGL J0922.7+0435GB6 J0922+0433?ïü±7'Ñ?3IЄ²B¤?:vFÇqt‡?3IЄ²Bž?ïý 0­t?G"៛ÅÙ?2þz"_Q‡?G"៛ÅÜ?ï×£_­¶"?tÂT""9?t.P)$îì?tÂT""9?ïÿ"˜x8Ù?$EO!ÂÛ?áñɽ
?$EO!ÅM4FGL J0922.7-3959?¾>˜ÕÔf!@ƋýϤÀ9sÒì¡~jÀ;ݸçì
@}"£˜öÜ@ƒˆ›D"…?¶hÛ¡%ÿï?¾¿Ïä.hH@Aƒùdo@Eìs±(¿Øæ4"E¿æWãa
áë¿éZ~›çQ³¿ã'ÞÑ·¿ì
ÓØZ¿ïÿƒmÞ)ìAGNfsrq3FGL J0922.8-3959PKS 0920-39?ïòPüÙ¸*?bo±Oé?[^L«±?bo±OéŽ?ïúiµ1?`Š,¸+Ë?FY+;Ãô?`Š,¸+Ç?ïjórJ"Y?Š?Ð8·?'¡'¶»´È?Š?Ð8µ?ïþ÷¯=?™gx†»?( …9Ï?™gx…©4FGL J0923.5+3852¿ÃvŸ»p[h@F½inX£/À9ÛýåsŒÀÀ<"æu@V¢NÉç•@ß09ƒ¯M?¹¡®æÝÅ?ˁR:Šj}@
¸e6»~@ÕÅCìi¿ÙÑãl'¤¿åZ:8
3¿è›!>>)0¿ê'?_†¶¿ïÿöût€¿Ênà]xV(AGNbcu3FGL J0923.1+3853B2 0920+39?ïàÉÛÜâ~?o¬Þ·›y?o6$#'L?o¬Þ·›x?ï÷¨â"Ê?jx´Uåk?P®:ÙÖmê?jx´Uåk?í»'õ6¦"? ·úS#?²#pVJÎï? ·úS#?ïÖvÂúÎ?b—nŠh?tóDž'˜	?b—nŠf4FGL J0923.5+4125¿Õ×â²V@F¼	ԕ+À9"+¸ënÀ<i3—Ý÷@QÞc£"@xAàu >?®<ÃÇ
–?²ºýíV/7@÷×ûÕ@
òÍtg†¿ËæJâ§T˜¿ÝOÍ¿å×6èÊYU¿äe8Ó¥"¿æÿe I¿ìÃßâSGAGNfsrq3FGL J0923.3+4127B3 0920+416?ïö†ãF€?MÚÀ†Ïö~?Rò9rÿƪ?MÚÀ†Ïö˜?ï÷°]§c?hRñÓÄ?PŸD±9Ðb?hRñÓ¾?ïÕ½Éä£R?vƒkö¤½?u!
®W?vƒkö¤½?稜ѯz?r¦"ZÓÔ¢?†šK"8!K?r¦"ZÓÔ£4FGL J0924.0+2816¿âÈFKðAÜ@F7ë¯#dÀ9î—ÁREGÀ<zãv\}¯@]ðáy@.þOü—–?¯‰N?J¿¦&ú?̞ª?ñlj	ÿ]@A<%J<d?îŽÃ|Áò¿äÒ8\gà¿èÐ"uE&¿à×J4¸¿ç>àæ_E
¿ä+"XÖ[AGNfsrq3FGL J0924.0+2816B2 0920+28?ïý¨=*·?-$ŽëõP?2¾ªDÞ?-$ŽëõÌ?ïýOe¤åˆ?MÍ©ePp?5"ÒØÓ½?MÍ©ePm?ïè¿Óù\?iüèÛ?g@ù,¤s?iüèÛj?ïþÌiMi¸?Õ~þ"g?#9k)dˆa?Õ~þ'ø4FGL J0924.0+0534?éaÍ.bÏæ@B#Bþ'Q~À:ô'ÛçÀ<ˆë"²'@ ,üÉÚ¨@â…Ãù¿t?©Ú—O¿¨é#šŽâ?ç·4Ã@	!'Ë?ïœd…D¿é᦮U¿ä³ñTk'¿àÏ;<1¿Ñ[=E@¿áãXàÿÇAGNbll3FGL J0924.2+0534RBS 0771?ïø‡j¿—A?Cë^àbè7?MâU¢ý?Cë^àbè?ïü_®~?Sż³õÈ ?=B$¸?Sż³õȗ?ïõê£=¼?Yžš¤þ'Â?T*¹"‡ã%?Yžš¤þ'é?ïÜö§´¸?^Ïs¬,Ç?q"¬?%¤c?^Ïs¬,Ñ4FGL J0925.7+5959¿äKÃè¢@E sÞ-èÀ;-Ówá¹À<àì^b‹æ@ ¤|Ö?þb7G"ê?Å1®ù¨"?¨ËPö½Œ?ä8j¤ @"Zî?ïòÆ@Á'/¿Ö–"'I¿¿á´b\Ô¿á[þ˜÷³*¿ÔOd!ȿۏ²tƒàAGNbll3FGL J0925.6+5959NVSS J092542+595812?ïþ8"وX?%I2<e»?,}Ògzn£?%I2<e°?ïý§–Âtš?HîEegë?2ÃIì[+‰?HîEegÿ?ïïιYT?j?ǐ?`1F¦«í?j?ǔ?ïî Û»•E?N¥Ñ›úw›?aß$Dj¹µ?N¥Ñ›úwŸ4FGL J0925.7+3126?ï/{6ì@F­"àÀ:…¥>éIÛÀ<«ªïê@VÿYfú@ƒ¸¡œZ?½‹.`ªS•?™€È½H X?ÚæÞP­Â@'4ð!»'¿ÒJÎZk†a¿àÜ.1k³¿ä±3¼Åï¿ØÞd$í ¿çáӟyØ^¿äWŸ#FVAGNbll3FGL J0925.7+3129B2 0922+31B?ïöÔ}
϶?RIük?RWä`—?RIüp?ïüÎtQŽ?PPÛ⎚B?9Œ_Us€G?PPÛ⎚P?ïëpâ_(T?p¢'¹þv?d ×¬C?p¢'¹þy?ï藢QÝ?S£ÆE"¨ß?gh]ô®$ý?S£ÆE"¨ê4FGL J0926.4+5412?àæ>®í7@F	š¿3‡À;wžYóÀ<؂ ×@ 6PiNù?ýÙ¤K¤CA?øh;ӕ¿?²ÛóÚ­¶?ðÁàŨ]@㉠þé?åë¡òYN?×_×Ár{ž¿Û·¤F›ÅÄ¿ÞqIþ7(¿ã ®Ì0ś¿ÕDzãíAGNbll3FGL J0926.3+5409NVSS J092638+541126?ïüêþÙ#??3$êRƒ0?8¨	6æR?3$êRƒE?ïüÌyHÖb?P}ïѯ'?9œ5¹Lçí?P}ïѯ?ïòÕ©¯'?dÉ)vAÃÜ?ZT¬Þ¡³­?dÉ)vAÃÞ?ïÛFNÚø	?YÉà^Cz¦?r\ؒƒû¥?YÉà^Cz›4FGL J0927.2+2454¿ëøëã<@F2wpyåŸÀ;0èÈ«ÕÜÀ<½{µƒ@*Wú½ËÓ@ ߛÜiù?ÑÁ‰7Kƨ?Æ#G'Ëvá?ó6¯Ž)ú?ù†ßúüá¿ïØgHðŠ?ïÿ¯"AôA¿åŽvàÜú¿ÐèkÄt8·¿ïûÆ«±Ê¿ãì5YAGNbcuMG2 J092720+2456?ïç¤0'YÏ?lÀzD?h[Ï}¦2¶?lÀzC?ï$ÅñÜ}h?­¼dDú€?›gAÄpRæ?­¼dDú€?î¡>iô¸?•š\z?¥ìn ´?•š\z?슈_¯Æ?©úæxÒ׌?»«½‡9Ë?©úæxÒ׌4FGL J0928.1-2035?í»¡Åm}×@5x¦—®ÞÀ9þç×NlÀ<c$—Žý^@ÐOo õ@Šúšeq?¸pÀ\Àº?¿å©érö@Ò}{Uá´@ºÉ,YOR?ïªFà!q¿æöÏՕɿçAȌÌ+½¿ç€Ú")=¿êï$°¹pÏ¿Ò/)"ä¤AGNfsrq3FGL J0927.9-2037PKS 0925-203?ï÷•ôÝú?L¤Ç.Øj?PÔEÖ
­?L¤Ç.Øl?ïû¡*&¢$?X:°WP?A{Wewoö?X:°W^?ïÁP>9¼?y¨2ê®Qµ?Wàûã!æ?y¨2ê®Q°?ïü>¦¯/?,¤ç3/q˜?>
ʆ‡"?,¤ç3/qv4FGL J0928.2-3048¿ÕH΀Æû@,éáŸÂ¨‡À:Rۗjë0À<(<˜6Ã@,LÖGtß@ùúÊ9?ÁÉõA‹¾?¹Q"º•?ö]‡ëlm@¿!"µ?à7Åü-ã¿å—Ae%Ç¿æü¥Øl=¿é6sXg¿ßc¼ÑG¿ïø*ÿ2$ÀAGNbcuPKS 0926-306?ïú@² ªÄ?D¿|tÖ?Fý7}Tñ¹?D¿|tÅ?ïù½°?i,U6·©?I	=½Š?i,U6·£?ïܵ7H…ñ?s¸¨Õê¯?q¥d[½Ñ?s¸¨Õê¯?ïØô·š?^""Ÿ³»þ?s…˜¼w2Ñ?^""Ÿ³¼4FGL J0928.4-0415?ÖzFxYÄ@?Ü_õHíÀ:"a‹5RÈÀ<oÙzZ91@vœ#·•-@Õ;f›Ö?Æ˃ ±P?º8öLÖó?ñÐD¡À›@	¥ŽÎºb½?ï¦pý™s¿ä2î4%¡z¿çe`!Ràø¿æc¤FÞâ¿ïÿø]ˆò?ê/†€b;	AGNbcuPKS B0926-039?ïý«¶89Ì?09ƒñ©æ?2¢N>1£Å?09ƒñª?ïüž,«?U-NÂ]ðš?;6"?U-NÂ]ð?ïæU9\Ç3?hÅýú?iªÆ£8Ín?hÅýú?ïë13¾?VšN?;?dÿÎíÌB&?VšN?;4FGL J0928.5+4048?Þ7Ÿd–*ç@G7žYò»À:ÝҜ¦šÀ<Âc:aûž@²Pt·?ÿÆ.¢<Ö?ÇYü ¤ü?¹1ÀíE"2?òB¸ý/¹@ z~¡Eµ¿àå´àFý¿æžã…uö¿ãk®Œp¿Øåøƒã¥¿ářœô—í¿ïÿö$´ë/AGNbll3FGL J0928.5+40481RXS J092837.8+404858?ïýàFV?-i ?0ýÏÕOˆ?-iX?ïüÖQ?U>^8¯0;??{O…|ž?U>^8¯0??ïï¯âQ<¢?h9Ž
&UÛ?`P®Ã]?h9Ž
&UÇ?ïÒ]Š‹"T?b?ʓõ…*?vÑ:º5Ö?b?ʓõ…%4FGL J0928.7-3529?ãÍú"3M@&p4 ½À:B ½å©=À<0d~.Ú@<gm!–~@ã`ݐio?»»žÕ(ø¿cD§"œi?¤£áÈÂ@ҐöÝÂh?ьPû"¿èKƒŒÚ¿â`c&¿à3Vn¡žK¿ç/Ë¿Üyh¿Ú/\#—^×AGNbll3FGL J0928.9-3530NVSS J092849-352947?ï¥ûåóÃÍ?€qžP©?†ƒ
	?€qžP©?ïöÏ"h|\?mE"ŽzË?Ra»/G?mE"ŽzÇ?ï°ÈͅYñ?Á€Õ¶›p?ƒÍ̞©"	?Á€Õ¶›k?ï¹®wI7?jº·4}™?"z"-²"?jº·4}™4FGL J0929.3+5014¿Ú‹þO|7@F¶™÷LÀ9Û~@w¿À<%êÅÜÃ@/Y­€@Ê%Ðt!?¥C'«¹µ?¢ó~½JM×?ûæ8^_
@ò{PÞë¿×R]šåÊ¿Ù^ØO·Î¿ãž"jc ¿á»ßá§z¿ßfÚ?&0–¿ënxÿQæAGNbll3FGL J0929.4+5013GB6 J0929+5013?ïüE·Ä?6ä
£??õÒG	Úô?6ä
§?ïü²,,*ï?O€j{/«à?:nžž¨†Þ?O€j{/«Ó?ïæ[ugPF?oÄ=–.:?i¤Š˜¯¸«?oÄ=–.:?ïúŽ4»?8jÂ.F«J?GÁÇ-÷?8jÂ.F«P4FGL J0929.3-2414¿î¦ÒÏ+Ü@3/ÃøôõÀ:úù€‰þÀ<›>»&²@~¥¢fr?ýTq÷" ´?Ô¿""Æ?Ùè'¯qr@  F\ä@b35e"?ï¬LŸ?ö»¿âåAã¥+¿Ôy;U@¤¿ã¸ÀÅ­¿åöü¿ïþöë"GùAGNbcuNVSS J092928-241632?ïιñ±ø?wÅ),Ãt¹?x£q§å?wÅ),Ãt·?ï¥}â‡~Œ? U_TÑÓ?† ‡^ ]? U_TÑÓ?틟(:¤?£ËYE^è?³£¾*ß2?£ËYE^ç?í²ÎC¡?—¾üÂÍå\?²o	Eâù?—¾üÂÍå\4FGL J0929.6+4621¿îB0×tðW@G
 r~À;"Îa!ƒÀ<"«ùiä@þžl<>J@|ïÅYb?Õìé¢Æi?¿·ÿãz?ߘ¶…7·Ò?øSƒ""_?ï£XK±¿èo~¹Å¿ã?æŸÜ©º¿ëBµþ,Á¿ã.¨TGñ¿ïùm¿¡9AGNbcuSDSS J092922.75+462046.4?ïösÙÒs×?U£öí¿Ü?SL[RÑ?U£öí¿Û?ï"|Œ‡1?¢Ë'6öÐ?ŽàÜÞ8³Í?¢Ë'6öÐ?î؎˜n)?˜W:Ôîˆ?¢wyk?˜W:Ôî‰?î$"âlŠ?RӊhËç?­·±Ù>'t?RӊhËè4FGL J0930.3+8612?éù󦀝"@="%¿­)™À9h›WûQÀ<Eyõc¶@MßÇPa@–£E?¶J¸ o÷Š?¸y/ýÚÇó@u5'Ì÷@ˆ¿6Œ.!?·ö*NçD¿ß·RDËâ¿ã7³`<οá²+–†¿¢¿é?qdÇ)ö¿ãcBZ£‹AGNbll3FGL J0930.2+8612S5 0916+864?ïøl÷'?q?EÕ¨kµˆh?NL!·>†?EÕ¨kµˆh?ïúËWuŠ?bç3r"	è?Dӂ¢)Ù/?bç3r"	ç?ïµYÂý¥Ì?€ìótìHð?'©@–ŒÉ?€ìótìHò?ïð:q›2¦?Lvë)G?_‹ɚµ³?Lvë)K4FGL J0930.5+4951?¦ËÄt%@FØwîN&ÕÀ:ÌÉÀ¨ÒÀ<È±µR@!t1¹áb±?ýP2é?Áǧ‰qX]?ƒMŽF@?Åö€û=" @÷ŒV:_¿àÕ¿ðEwÙ¿ä<ôb=ú¿ãooŸ?‹¿ß2ù<†ª¿Ýnm[x Î?«Á^¥…iAGNbll3FGL J0930.0+49511ES 0927+500?ïþÌóŒ1D?]Epa\`?#0Ç<ëÁë?]Epa\"?ïýá9/Ë\?H¶¶¸$/O?0ö6¥
?H¶¶¸$/R?ïú©0–é(?Y<Že,ÆÏ?E[=¤[]—?Y<Že,Ƴ?ïøË=íÞÄ??¼Œ‰ Š?LÓH"ó??¼Œ‰ ‡4FGL J0930.5+5132¿ç¼j-z@FªJ¾j3{À;¿°ä8úÀ=u=™¾ƒ@ D߀®'"?ü¶¦4²4?ҒߪJ?Ïv³»ƒÏ-?ûtÓçsA@@¶©
оt¿ßÓ^Kå± ¿ïÿ\‹/ô?ïüSme^)¿ã;§««¿áÓÌ/îÛ¿ïÿþó…õAGNbll3FGL J0930.7+5133NVSS J093033+513216?ïúˌ¥µ×?C¯c¥çY˜?DÑÍi(Ó?C¯c¥çYŸ?ïú%[:H¢?y}ÐSU"W?Gj"݀]?y}ÐSU"U?ïjêÙěP?Œ[·æ=ýO?'¢¤Çl–+?Œ[·æ=ýN?ïÕÁ«'ÿ?c¼"aà?u*l Ê?c¼"aà4FGL J0930.7+3502?ßå뛐n@G`ÉÀ¨ÒÀ;0f('ðÀ<ܾ•Òd¼@ÜY·Vmö@+À nŸñ?É?æPl?­HPÑ©«`?ã"cßùOb@î¿æµ?ïê"Q€ü?·ÌZ ²Òü¿æòƒàÊ°"¿Ð]ãŸ''¿éÔ+{¯¿ïøÿ?æŸÝAGNbllB2 0927+35?ïߓqšº?mù¹ëvÞ;?p6G}²£??mù¹ëvÞ@?ïñ툘€¯?p¨¤ÿðáj?\$îÎþ¡›?p¨¤ÿðám?ïwìr¿Ì?‡H"@ï?'q¨~§?‡H"@î?ï7›a-W"?…*RÄíeo?™"ÚU
—?…*RÄíep4FGL J0930.9-1015?¢D፮ũ@<µ?á—_-À:Z'¹hÀ<vö=Ÿ@æF×)òî@WUÿæՍ?¿]ç;ãÛÝ?´zr!…‹Æ?ñ+!Z³@ê$O?®?ïÿÕ%t.¿ÝÜxüÁE¿äŸNyà–®¿édŸ;ïð¿ááHtEL¿ïÛþ~ÀAGNbcuTXS 0928-099?ïÿj³ŒÔ?ίvpä ?'©Že|…?ίvpåR?ïýâü	?Ø?G®Öø?0è¶Aù?G®Öö?ïØmk¦=Ó?uMjïp @?sÉJ,áƒ?uMjïp <?ïûïú»?1Á›j?C°@¶$?1Á›p4FGL J0930.9+0033?çn~ùºK˜@AŽ'bEoÀ9›õœÏ®ÿÀ<G^ñýÞ¾@L°·mj@Ƭ!\?µKÌ ñÁh?Áö*¿@ƐšíV°@ÿ÷ªÖ¿ÉjW·¡íP¿åþŸ­¯Ñ¿é­'©èò¿ë0߁w^¿ïÿØþ3w&¿ïØAªÅ;AGNfsrqPKS 0928+008?ïöØ²bŒ?UÄ%WO?ROæ›:æœ?UÄ%WH?ï2Uçñ?±›Îv	ƒ™?™µCß==?±›Îv	ƒ™?ï°o"OY×?€i
qÅ}?ƒä7l)Š˜?€i
qŁ?íÍÃٟ2½?Ÿ
8ÎÙò?±'á3j?Ÿ
8ÎÙó4FGL J0931.2-8533¿ç_Պ"ÓúÀ8:dž;îÄÀ9ÏÝ;¯ÙwÀ<H~@WZ¶"áÒ@6Øôù;Á?´4T_AÉ?™òĒZz?ã[é4â`@Û3¡íûñ?ïðDÁPï¿áŽÉý³ø¿é•lä.é"¿âÒ5!Iü£¿ê';ÿŠ;¿ïÿÔ@ßn:AGNbcuPKS 0936-853?ïü‰ýµ?4D½H¾?;°/òbD?4D½Hµ?ïþfÛ>K¦?Hÿ{mŒ?)'LE²?Hÿ{mr?ïÏ
/†MÓ?u,ˆa'?xyh<Ù?u,ˆa?ïýI²ÐD?'º€RIJu?5²l}Þo?'º€RIJµ4FGL J0931.9+6737?èÒ2¿[]@Cåwž™À9õ*8¸®2À<Œ
¨y0@¦Pç}@ïw݇/?²õçMVŸõ?¦ã,Š¢…Ñ?óŸÁ?/Á@
¡–‰ÄºZ?ïÿ·ÀÌ
Š¿â¿a!-!¿å1ß«Ì¢¿âß5…¿älɌ¦l¿ïmŸ`=AGNrdg3FGL J0931.8+6739NGC 2892?ïýnWuP—?.K·äP#~?4DU{A ?.K·äP#¾?ïüìW6?PA¬?¶?8FOÏ9Ó?PA¬?º?ïîÍ{Ž*?fÕ±Ð=Շ?a2"qäÕÀ?fÕ±Ð=Õ~?ïðfLƒNÓ?Iéä	'¹e?_3fùbX?Iéä	'¹U4FGL J0932.6+5306?ï¥v¸ù@F ÇŸfb5À9¡®×€*À<‹íóŽ¶@b9®øP‰@/ÜÌõ?¯S¾Ãõ¶?µBJ¨DØ!@Â;C¢ìÿ@†Èg¸K?áÍaýËó3¿ãÑG»€t/¿æd2Dꁿ炞«QR¿è7·6¿ãÐ9h×YïAGNfsrqS4 0929+53?ïýÀV4ˆ?)ÌݍFB?1ýN_CºÃ?)ÌݍF|?ïûßÀÝ
ê?c,ß»7©?@€ü‹ÈVð?c,ß»7¤?ïˆ9'@?wܔ¤ƒ<?z<Àcl_€?wܔ¤ƒ>?ïÿœ'W3¾>û H°y¨?Ûj3C+>û H°vÎ4FGL J0932.7+1041¿éBe·ñü@DIÞ½çÀ:ñŽd²1@À<ŸN"
@ /¤¨ìGç?ûüÇÓ¦Ü?Ì" 3§!?жIÿj.@S¥Ýt»@GmÑi¿Œ?ã[}i¸*~¿é˜¤ Üš?ÐÓۉÓÿ¿ÍøNñ¿âÝø©Êi¿ïÿ£^ilÖAGNbllNVSS J093239+104231?ïïökø˜?Z)ÉÞ}?`	"gàç?Z)ÉÞ}?ïöO?xG±~¸ÍZ?SãÁaÏò?xG±~¸ÍW?¨VÓ?ˆ5m‰ò£?ŽÝ•ê\‹m?ˆ5m‰ò¦?ï
ãÌ…ö?"ää­Íކ?žCŽFoA(?"ää­Íކ4FGL J0933.5-5240?âM''7¿åÇòÝ؍ËÀ:Ͼï"xÀ;È$g¾U;@!B<¨§Ôp?û´ò»sÞõ?Îß$}¸½v?ÑhEƒíµÑ@½ÞÎW@U›ÛhF?ïeû7Cc¿é MÈ௿ÜÒýhv¿Ù6ªK˜"Ç¿Úó­¡¹M¿¿çÓșaeAGNbcuPMN J0933-5240?ï%­AÓ
z?™"Òú"+
?›JWŞPõ?™"Òú"+
?ï0ì¿ãù?¶'E ?Yâh€Ð?¶'E ?éÿn2òÉ?±[Ø´µ›®?ÈG47üß?±[Ø´µ›¯?îpöCx?˜·sƚð ?¯ÈþЛȋ?˜·sƚð4FGL J0934.3+3926?䙎ë¿L@GÉ-ÀÊ`À:-ŽÚ"ö¥À<‰ì©&¥@}ÈoEF@i3]$žE?·3Øõz?Ž8èÿ³T?ÓþzÄÂ<@É"ž:"$?ïýqåöi~¿ä\u¡Â²í¿æɨnZQ¿â¹Ùె¿æöJ²È¿ïÿø¨ó©°AGNbll3FGL J0934.1+3933GB6 J0934+3926?ïý?_C¦?@ÓçNËp?6ç"Þ²?@ÓçNËj?ïûìÛC}?XäZœ?Q"?@L"Žò!?XäZœ?Q|?ïãª/X–B?r«êÝ?lUЧi½&?r«êÝ?ïÎëº0?dJüy4g‹?xŠ"ñqçV?dJüy4g"4FGL J0934.5-1720?ٙ۱¶Í@8ÃF4—·AÀ:åV"tnÀ<__á'@ 됚—?ÿ%"ü|?ÇÂЊ¢H?°³¢?–ª?îïŸËm@­Åñxô¿ÜÈ'ç%"¿êõŠèü®?ïþ@!Ù¶¿è³2ÇÓi¿Û,kãþ"¿Ñç6žË2AGNbllRXC J0934.4-1721?ïüuݯñ­?8ädc®v?<Q€rG?8ädc®vd?ïüMËÐú?Z#A~N°?='§ùx7‹?Z#A~N¢?ïÞ 	p¹?t!€Ï*Yt?pø/ûG£Ä?t!€Ï*Yp?ï³
˜?vSá<§?ƒ=~Yÿ?vSá<§4FGL J0935.3-1736?æOv+Æv@8¹'^éšcÀ:GäB4WöÀ<2Ÿèh3Æ@!mQ³¦á?û®Ð³Z§?ÄoH7QOÿ?º¢žA-?üG*{Ԍµ?ÿ·Æñ¬¿ïkÚ佄Z?ïõeݪj¢¿í†òÞ€é?Öª"XŸÔ¿Ô¾B%>}ê¿ç:R ß²AGNbll3FGL J0935.1-1736NVSS J093514-173658?ïê§N;U?gÁP}(?eXþ±Ä©H?gÁP}(?ïÓtÅÀ‰Å?¤ì΂éa?vE»°?¤ì΂éa?ï>4A7·ý?'p…0Œ©?˜9wÙ	Y?'p…0Œ§?ïù-Ï|?É.Fçp5?ÀÚ\fž?É.Fçp54FGL J0936.3-2111¿ä.¬(þJ@6už×ÆûÒÀ:¿YHp²À<iéæ¹@ é#mîE?÷ d#–?ǚ¶Äø˜?ÔÛ:£¿ã/@¢HåL"@E`í²v¿ïÿýF\I?ï÷{+ðHÓ?ìäS äQ#¿Ñؗü`Ž5¿×<ü_·u£¿æåÂ!øùAGNbll3FGL J0936.3-2114TXS 0933-209?ïÆk©ëd?ùuÌ'5?|Ê+
MòŒ?ùuÌ'4?ïé<OOh?~(m€Vtµ?fÃá°°–´?~(m€Vt¯?í@öCR¦?¨+"=&G?µøMçýjÓ?¨+"=&H?ïX}H\õû?"}‰"ƒüQ?"ðVôa@ˆ?"}‰"ƒüQ4FGL J0936.5+1847?äæ™/´2@FR  ô×®À:®4|ßN°À< …S'wŒ@ÁÕh|Á?þ@¾kàùª?ʊÄê€;û?Ã*[]É´¿?øJÚ3½œ®?ù¥HÇD!Ã?ë£t'ˆÜ¿ê7N€–"U¿Õýu‹¿ÜžŠD<
¿ëP.Ë¿ª°#çF¡AGNbllGB6 J0936+1850?ïº]Våô?…»Ù!ý??hª`ƒ9?…»Ù!ý??ïP8q$ï?¢WOCh?•øñÛb?¢WOCi?ïTg)K?ŠÞ…±ñ7?•sߜÖ?ŠÞ…±ñ3?ìVbgNo?£/=j´;?½LìÃõŒ…?£/=j´;4FGL J0937.1+5008¿ä†²?E Ý@GVºI<‰ôÀ:?'Á^ÁÀ< *#¿ø©@ GÏ!É@z䢬h?ÁS¬åÑ«"?ƒåä¥@+e>H:+@
žÄ½B?í´®"%â¿âÀ_×,v¿åš9҉¥0¿å݅TÖ¿ïññ\Ï¿ïÙ§'æøAGNfsrq3FGL J0937.7+5008GB6 J0937+5008?ïÅ8¶³j?€E%.]Ù?}c¤ò&J'?€E%.]Ú?ïø·H~Þ@?cø¢5íï?M"Þ†üù?cø¢5íç?ïõ"·?"v´"MsÜ?íÿ!Oi-?"v´"MsÞ?ïÎ5Ï{`?söLC•?‹ÌrŒ!(?söLC˜4FGL J0937.9-1434¿î¥ÒP(Úw@;7Ffìž#À:v^$x…MÀ<o»^æ?e@ 
Õö›þ?ýæD·%?Äú`XÛ8u?Á¤÷Ãpƒ?þXˆøa¦
@
ä"¬¿î¶Ãvö?ï÷uýÞÄ¿á"&ÈÁ¥Q¿à8äl-P¿×oXz™¿êá´N_ßAGNbll3FGL J0937.9-1435NVSS J093754-143350?ïýeˆÓS?5ÈlSŸá?4×ó¹eh¿?5ÈlSŸ»?ïüÌ6øtk?Xô¦lóA?9žH<\­b?Xô¦ló=?ïܝºUmI?rK¢ <ÿ%?q±"ÕI[	?rK¢ <ÿ!?ï÷®cøç?B||¦ÚË?P£9æ5h?B||¦ÚÊï4FGL J0938.9-6403?␚®W²À!AMµ•x£À::Þ¨—c^À<;0µªq@?Ôó@@˜Ž¼ÆÅL?½ÊA¤åþ?­â~ðå ?ðXÑRm‹@éØÅ~yÙ?îˆ|:䝿äžr£hû¿áV™y¹*¿çôÀfŒý¿Öý'aĖ¿æµ¾§6AGNbcu3FGL J0937.8-64071RXS J093850.5-640334?ï÷*۞"
?OHŒP³£f?QªHÂÙê†?OHŒP³£j?ïý	œ&ø?Ypˆr;?7·KÈ5?Ypˆr5?ïæÌéŸ?r?'Ô6º€?i¶2a??r?'Ô6º‰?ïä±
öÈÔ?U¤³1×õ?kNò	7+¬?U¤³1×÷4FGL J0939.3-1732?ï¶=ñ͇@9yØ¥H#…À:
tÓ³¬À<Yõ2F¤@œ' PíÙ@'%IÆ?¼µ¿êç!?½Å°"òô)?ÿη«c@ÙÛ]3a×?ïýCWm¥¿å©?Êjå¿áÒ¯')c¿äKùӖª¿æuQ@9¿ïèÎ?ézAGNbcu3FGL J0939.2-1732TXS 0936-173?ïýΧf*?9—é‹
i?1ŠÄÏ>²^?9—é‹
i?ïüТYêÀ?P*†aÊõ€?9zí0©ñ8?P*†aÊõ|?ïÛÉäf£f?r'**Nq?r
Ì®M	?r'**Nm?ï÷qõÑN?:–ÿç+'M?Qü]d#?:–ÿç+',4FGL J0940.0-2828¿àԜ¨9$@1éi ­ŠÀ9ùÓ°ìœvÀ<3ÅìÞ»@z[±×~@£ŽDÑÁ(?¸f¸³?ƙ˃ ±P@Mí®Ä¤	@Euà¬Óˆ?è]ÿÅGN¿ä` CAs¿å"—Ú|¸¸¿äy;.ª7¿ïþ—J4¹?Â<:˜Ø(¡AGNbcu3FGL J0939.9-2831TXS 0937-282?ïÛC^Õô?qìǨî7g?r^P•ò¸?qìǨî7g?ï÷ï
ÇÖ?h–<àtM?P!ëÀpRÔ?h–<àtF?íü|G1!i?¢µ°¦*0H?°Ævô½?¢µ°¦*0G?ïöÚb5f?A¢È{¯ßž?RK;•ã5,?A¢È{¯ßž4FGL J0940.4+6148?æ|(͊Z0@Eš:э%îÀ:ž:'ÌE¾À<œl%Ã(@ ÿƒ'ǁ?ûþ FÇd®?¿[äØ1Yê?²ùÞÓµtA?ôʇx.æ@jk5Øÿá¿Ü¡]Þ,›"¿íNj¼[f¿·Ãñ®¿ÛiÝk폿æx`ˆ"?Ç7¿)ÌAGNbll2FGL J0941.4+6148RX J0940.3+6148?ïÿk7ÿC?ùJ'‹?™·''?ùJ'†?ïý_EÈ?OP"Uk?5•Ñ¿.æ?OP"UH?ïûžÃ?[ÎéF?Cҗîœ?[ÎéI?ïî"@û'[?Rd¼:îÜa?a{¿Ø£â?Rd¼:îÜg4FGL J0940.7-6105?ä¸Á'"À!)Es§˜À9èy§‹Ê¤À;ڽۘA«@—Š«j&@æc[ïêß?ÁEj˜?Áâò=ŸÀ@;†Eÿ¾'@	C\($¿ÝÇkäՂ(¿ÓENJm¬¬¿æ}å=ÜÚa¿ç¯žˆì£,¿ïicÁpx8¿ïÿú@ùDzAGNbcu3FGL J0940.7-6102MRC 0939-608?ïáÏrõƒá?mH´'é?n0
|ž?mH´'ì?ï݇݊?'=|mÀsŠ?qp¼:¹x?'=|mÀsŠ?îl¶'é;x?œ¶Ñri"î?©4—ÑlH‰?œ¶Ñri"ì?ï>UsRä?ƒºa2-W?˜5Q•¾ã?ƒºa2-W4FGL J0940.9-1335¿ïþLBÜá@<lӝ¡fÀ9œÈ\ûƒ™À<'Kžd¶@üËÙ1ß÷@g'ûÈbÛ?²z|öê?½iIśÖ
@‰—Þ®v @¥o;¢?иœ>9¡Œ¿áŸ=ب£¿äNô‰u_¿èWÿ›V2¿çþîк˜¿ïùö€û=#AGNfsrq3FGL J0940.9-1337TXS 0938-133?ïý`Bék?1
-0Vþg?4ýè·$ŸÉ?1
-0Vþp?ïü5v8ò?T(—Í¿@?>WN8zº?T(—Í¿B?婢kàóq?TG",ºb?…_åÃ#¼?TG",ºe?ïý¯SF£f?"8ÀÒ³MS?2…eÊäÅê?"8ÀÒ³M'4FGL J0941.7+4125¿â×XH).@Hp}€^_1À;@·E|À<º¢ô§@£Nçï'õ@q<ƒ>?מý0ÂÁ?å
ƒç€­:@È[TŠœ@
eBŠ¿¿ïë"ÌÐþ‹?ïÿì´É È¿æ/ñ)£gy¿êOž£Ä•Ç¿çõ2F¤¿ïü¾â©WþAGNbcuGB6 J0941+4121?ïPû_q?'Zxñëü?‹ëÁ(8ãÐ?'Zxñëü?ëBßÿë¶?͹>¼X?Òô€Q(?͹>¼X?êC°•.[?°@Cá?Çêñ=«F'?°@Cá?â6J¾‹É¥?À'›€û±¥?ۓj'èl·?À'›€û±¥4FGL J0941.9+2724?ï¯C㊚@HëC,¥À:<éhSÀ<Œ_Æ94Õ@ûˆ÷5=@-'$ZR\?¹ùÛßËhZ?¸r*rD?ø§{‰äð@	É0àóu?í ¶ž¸¿à‡)T ¿å:óṘè¿é£L Â'Ç¿àn—Oß¿é$Læb AGNbll3FGL J0941.6+2727GB6 J0941+2721?ïü°Øšß‰?AØzõ¶+B?:y;)µ?AØzõ¶+1?ïû€4á\b?W:9¬<Œ?Aÿ,zŽw}?W:9¬<†?ïå|ž±Y?mtxT?jôƒaN¨z?mtxT?ïÉW6XT'?hŒ˜Áˆï?{TdÓÕ¾õ?hŒ˜Áˆê4FGL J0942.3+2842¿ÇŒö;óM@H<'RT`ªÀ;D€'q^èÀ<È<){úL@ ¿›7©d"?þ,7«gø?ÆViGt‰?‡ºhµåÄ?Å_<¦y{í@Pò‰ø¿ãù`ÃdC¿àÆv;Ƭ¿ãÈßëb¿×:,âMf¿á°@¿ã°>¿ÔýAßAGNbllNVSS J094223+284413?ïþá|X?!»ÀP‰)?!è>þJ"?!»ÀP‰*?ïý¦z—!?JÀ†ç?2Ì+G~ð>?JÀ†ç™?ïúz+›Á¾?F8›Í|?FQùa?F8›ÍC?ïúÕOB)¹?2—&#K¨?DªÂ÷Y‹?2—&#K‡4FGL J0942.3-0800?±황ØY@@'1]pŸÀ9—2éaX
À<^6=@e¬|`C@ç¡di6?³m0/Î?Âu'ÿ ±ü@AÁÇ@£$fˆ ¿ÁgncµÜñ¿Õû"¿e=¿áƒ^nË:¿ã@*'zÁg¿åb¼ù2±¿ïúÀZ΂¯AGNbll3FGL J0942.1-0756PMN J0942-0800?ï÷ÞiÐ5ñ?LýmI½®?PC,_"Î?LýmI½®?ïû¡&`?Tª­ko¦6?BÑ{f'c?Tª­ko¦3?ïEædVK?Îñ֓:F?—C3u<ö¸?Îñ֓:F?ïú"jòpH?1¯m,@&?E²T6>áP?1¯m,@64FGL J0942.7-2028¿îUö^‡ÕÁ@8	WG²JÀ:Ö½A>Ž±À<'›Ø'@¥:=h–A?þ£ð4°áµ?Æx»þsc?¾iAžA/[?ø²'¸#È@ÿŠÏ§G­?ïîá"Úíø¿ÒwØ¿cm¿Ó:4g¾€¿áÄÏ9°%¿ÝÀ¯óx2A¿åÍôIéXAGNbcu1RXS J094237.9-202720?ïûYåò¡ñ?G0˙ө2?B˜h5x?#?G0˙ө%?ïü=ͨK°?_7ðlzü?>'½¢{¬?_7ðlz?ï䈔8ó‹?tcö_$"ˆ?kwkÇtå?tcö_$"r?ïÄïèò…T?e‹î3?}ˆ†½V0?e‹î,4FGL J0943.7+6137?æ -rº(Z@EÑ(9-ŒÀ9ý,ðùÒ¿À<q
À²ã@íúCR@Žm=ðüW?´ÇV2ç‰?Œ.·´è?Õ¿~°Š!@Oš¿ßS?ë]F,4;q¿Ýq¹`‰W­¿éOt.©6¿å¹ôMDVq¿ïÿøãú?íÑØÀ  AGNbcuFIRST J094420.3+613550?ïý%ˆ×?;à }–«?6Ó¹D"?;à }–ã?ïýó¼ÎY?KÑ lS?0b‹õ<#?KÑ lQ?ï™8mà¬w?†—©'*)?‰±ä‡Ôâ@?†—©'**?ïýiò£OÓ?*‡³åêÆ?4°jåfó?*‡³åêÏ4FGL J0944.2+5557¿Ë…»·é'@FûŽ\NµpÀ;q¬O~ÃTÀ<üóæIî@—wȹm?ý–¡G
Ë?ډµ@>3—?äûë~Õp@—ÕÄÃ?ñðtY™#}¿ïýv:ÂÊ?ïÿÄ}îB¿Þ¿EE•6¿ámžÔký¿ï°B¿êfì"¨vAGNbllNVSS J094441+555752?îڙ"îhå?£–^hŒ&ß?¢VfÁqµ?£–^hŒ&à?â¨e*Í^[?Ö¹íéž?Ú¯5ªeCI?Ö¹íéž?ê—ó
>?«.¥0ÑxÈ?Å£°3˧?«.¥0ÑxÈ?ȱMlB?±"= À?éӜ¬¤þo?±"= À4FGL J0945.2+5200?ä1|½£Ðƒ@G´"ÀÀ:YôNñ՛À<•Ìe÷@»MôU@Üʵ›?ÀÊóÙ¬T?ÁÛÕ~L69?ú˜¸É	Ê@[q¥ß£¿Ôlbñ¼Æ¿äˆ ËQ¢Š¿éx° œB@¿í•Œßvó|¿ïú¡†Íäû?ïðÝî]@MAGNfsrq3FGL J0946.2+5209WISE J094452.09+520233.4?ïý¥¢"°ú?9BoLÛQ3?2Òîêx*ü?9BoLÛPò?ïüŸ«ð&?Y¦F_ՏØ?;ƒ ~Ìõ?Y¦F_ՏË?ïÐ(½Ô÷?wƒââÉ]ß?wëø!"ì?wƒââÉ]ì?ïúiSŽ¡?<Ä1n¡?FZ±Ç¡~l?<Ä1n§4FGL J0945.5+4635¿è=®ž ž@Hf¼b~À;åác\ƪÀ=—^Uö­@!ÏÎ_IÀ?þº©êIµV?ÅŘ•2¿¸9ë‰%ƒ?í–?aê«°@!¼:®Q¸?×A¦=–ä^¿êWvßZn¿Ö·¯™¶¿å®ùèŽÊ3¿ÒS^a_@'?ÍãEµ÷AGNfsrqB3 0942+468?ïüòîjb‡?8üM?ëóv?8hŒ¬ëÑ?8üM?ëó?ïþ­FŒ?Cf×WmÙ?.•+Ÿ(Ã?Cf×Wmä?ïëì:}Î?p¿Åª'üý?díł0_?p¿Åª'üú?ïöBvD‰?IPiÁw8?S{ví½f?IPiÁw14FGL J0945.7+5759?áYÆDâ¹@F±3 @|ÈÀ:Âð\À<'*¢jùs@[êæhTR?ýþŽæ¸0^?Ãëv?Úá?Í5³Ö†´å@üŸS @
…ÊúåŽæ¿¹)LÕpµJ¿¼µ,òý8%¿ØR'_js¼¿Ù;}8ºÝ¿épà"&þ¿ßVóé	AGNbll3FGL J0945.9+5756GB6 J0945+5757?ïÇñ‹»²n?z­Ž;E4¡?|:"&É?z­Ž;E4 ?ïû%BüÊ?X'"Y³%Ü?CjôØñ?X'"Y³%Ö?íȱFœÜ?¥GnЇ!?±ºuË:?¥GnЇ"?ïá"bÊ"?V¸"³ÇÆû?nbݝ5ݍ?V¸"³ÇÆê4FGL J0946.0+4735?âÚEvíãº@HW<ÈóÀ;ŒDÄU/À<ÝêPkR^@ ¯7eœè@ËHZ⤥?ÁY°àÝûÉ¿¸ö·Au@I?ùìÅÛA?óc-+²5r¿î~¸—·¿bø;v´Îe¿ê½¦îí¿ë_:øúRA?Þ]JÿÓ?¿Þ3xgðª"AGNbllRX J0946.0+4735?ï{
(/13?—¬À_îãÓ?žºúÙ¾?—¬À_îãÓ?ï',­—Y?¬3¸"…Ú?‹´Ôš>©¿?¬3¸"…Ú?î—÷/<;G?‡R&¾û?¦€<Kš?‡R&¾û?ï}(‰B¯X?Œ/#Àßñ²?Zîתò?Œ/#Àßñ²4FGL J0946.2+0104¿îúz[eV½@CH
|ZÄrÀ:¶ßh°ÄÀ<[@dtß@!T)΅‰—?ü‹'™Ù?Ëùwœn¶?¾Ö?;‡?ô›ƒEW"@¤}M]«Ø¿éo»^g"¿ÝÕÿ™'Ú¿ämð‰Ó©¿Û'/'y—q¿¤ûg{¯¿é˜=‹ü£AGNbll3FGL J0946.2+01031RXS J094620.5+010459?ïú@Jöî?I}ÏÓ§}?GöþÔ$F&?I}ÏÓ§ƒ?ïü"¢'Ù|?Q§ùÔÉ?;Zëi4Ä?Q§ùÔÍ?ïâ'ï•d'?r»€"Zç¥?mmj›}"?r»€"Zç¨?ïÜüþ†&?ezGJ5?qö€¼í8?ezGJ54FGL J0946.6+1016?×=8p»"f@E·<³åu:À8†'M!À;ק{¬]@æP4JàN@ÀÐ$p!Ñ?Ÿ|/Ùêö?´Û³@^çßwÊ<@´Çç4×ù?ïо"$哿àð´"†è'¿æ—ºÁÝZ¿çlÏ¡"c¿çµ:uFÔ¿ëëJ ŠAGNfsrq3FGL J0946.5+1017TXS 0943+105?ïý`èÿü"?-‰ï·~Æ?4ø¸ãó?-‰ï·?ïøyUOr?bªø«êD?NªÃ†1b?bªø«êD?ﲶC5öé?€ÀÃ{¸·g?ƒRo2'Eš?€ÀÃ{¸·e?ïùHïÇ<È?9,%ƒj+?JÜ@ãßð?9,%ƒj44FGL J0947.1-2541?Ó|ïk~–"@5Ý~Ë·úÀ9cf´iÿxÀ;Üå`A‰7@Œ•]õ©?üɕà§?°Xù:>?¶w%ü=ÿ@
'¿}Xñ3@
9¨…oÁ?ïò'x=?Пà·õ¥¿Ô¡â=wYÔ¿ÞgÚúâß´¿ÜÕÓ;{׿à 4éì˜AGNbll3FGL J0947.1-25421RXS J094709.2-254056?ïùmA:ç¤?H¾ÝE5c?JJûar|?H¾ÝE5f?ïäÉ=&ů?€ªe¬Ã³?k6ÂÙ:PÈ?€ªe¬Ã³?ï´×Ê,—?"‡1蓮?'Ê8MtÙÆ?"‡1ï¦"?ïuK†EI?tMióá?'\֏7W?tMióä4FGL J0947.6+2215¿Ðüœû"®@HJƒ±ÐÈÀ:ðë€ìújÀ<´¹‰$@µE@ûZ~ї?˾_·¼^?Ðe)O"¢'?ÿý&g@Úp'ÉôU?á΄'Ai?Ðgâ<u§!¿à"Ä"ïï¿ã´zÆo»¿åˆ©©µ¿î•³€ y]AGNbllTXS 0944+225?ïáâRM?iîôÞµÖ?nëü­²õ?iîôÞµØ?ïú‰ ›¶ò?Zs༗?EÛ}'$9?Zs༗?îÿ>6VQ?"W7?m? Üššë?"W7?m?ï'y'É?sl)7§Xp?a¸›M¼î?sl)7§Xr4FGL J0947.9+1121¿æ­O«ª@F¸ºÇÀ;n'D:ÂÀ<›@'§@ »;'HnY@¢õ}Åþ|?¢#€ã•;¿¾Ìô9ù ?õò-å˜î@Ó£¬íßA¿ël™ñ®-¥¿æo"‡¹E¿éÍÝ~냿ÕòŒ–›¸¿ÕmË"°¿â=v:ÂÊAGNbllNVSS J094746+112020?ïûs­Ê=??ÉqŒª?B1H×ã??ÉqŒ¥?ïý¤á(¬?MŸ¼Z:?2Øóöº™
?MŸ¼ZL?ïìµGF?u$¨Ý»Æ?câJ渹 ?u$¨Ý»Æ?ï÷FÇA^r?Gw#+T\Ê?Qrq}C@?Gw#+T\Ã4FGL J0948.6-0338¿Ñ;ƒé©V@B!ؾr–öÀ:ò6†¤ÊOÀ<|›U[|(@¤L9µ@R§åŒ·3?ÃéùÃÐϼ¿¨ªWVþêV?áõbLM@~á8>µÈ¿à0(QWáh¿Ùgð>Áܯ¿éÕ2ÌÛæ¿Ûà?:¨rz¿ïÿÙ3ã\[?ï¿xPs¶AGNbcuPMN J0948-0338?ïø1ZâF?PÊI…´›É?O:— våÆ?PÊI…´›Í?ïý(Åî ?[NØãp"`?7¾¹ÐŠý˜?[NØãp"l?ïÀ_Öö'ö?~¸‡¦·V?Ð"¾…¸?~¸‡¦·f?ï÷µ—±`v?BáÒÎW­·?P"Н?5?BáÒÎW­°4FGL J0948.9+0022¿áìCrIGv@C[¹pޏÀ7Û:,K¸eÀ;ÅÀ–]¤÷@~jM¦¦ó@Ÿ¬EmÈZ?œX¥f4?Å&J*øQ@$»`Iì³@O­·4¿ÑA¹my*¿äz™ú©¿éšñB¢çÌ¿êÐ3¿J-K¿îÇ·ºã¿ïÿ&¼,k™AGNNLSY13FGL J0948.8+0021PMN J0948+0022?ï"04‰?"~øM%œ?Žÿóÿ2ÝY?"~øM%œ?íâ.zœã³?Ã¥ Uü,ó?°îŒ+âk?Ã¥ Uü,ô?ítNÝÙ	?«%k°:±?·¼]‰7À?«%k°:³?çˆ0Œ?»›f
àŒÞ?ÐïŸßÜè?»›f
àŒß4FGL J0949.0+4038?Ø-ÆTeøŽ@I'½{ 1ÏÀ:{ôšq/îÀ<âž43@I²dkº@ñ^aµ&¾?º7U½¿"øæ'´?ÐðjÌ&´ @¡ïDÆÙn?ÎòŠ÷jZ<¿ãZK:õ†¿ë&qN õC¿ãâg3B¿ã{.¶Ì°¿áäúÀûÞAGNfsrq3FGL J0948.6+40414C +40.24?ïúÐ9™¿u?BHöL?D¿™*u?BHöL?ïþe‰<Ñ?Dzl‹á¹?.™§l2ãQ?Dzl‹áÊ?ïâb§†™Ì?o×Ê[Õ¿Z?mXyf3¿?o×Ê[Õ¿[?ïüµŠ¥Yf?)8•·fVf?:SªÕ4Å:?)8•·fV4FGL J0949.2+1749¿Ø/&ûPŽ@G'«!ZÀ:Â㨱d'À<ˆ–&G'f@<ÁQnˆ@öå¥
ç?Å.Bž
A¢?Œ$P
Öϧ?ÂèyfkK@ø÷2Q
¿ì]ÒC.S¿¸¯ƒ»¶Ð¿è¸5›Ã?…¿àó›}Ê[-¿ìE¶ù%ñ+¿ïÿÉ–oAGNfsrq1FGL J0949.8+1757TXS 0946+181?ïúõb¾vL?Gt±^¿gª?D*u&Ó×?Gt±^¿g§?ïýÿb¾€Ü?G™Ú3†Ç
?0êù%Q?G™Ú3†Ç?ïa>£ d?ˆ-#¤q?‹ç°W7æß?ˆ-#¤u?ïý&BÌÇ?)"ɹC"&?6Íé™ÇØü?)"ɹC'Ù4FGL J0949.7+5819¿Æùy˜h¬@FÝ]Ý*èâÀ:=çi0EBÀ<x5k×Í@Q¡?*bT@Î=EìÏ?º"tôô‰)?¶ûOþ+OË?ørÀF¬Œ»@zùdZr'?ÜÀÄÖ´,¿ãG(é-U¤¿çkÄߘl¿ë[î¾96-¿Þ¿â®‹n¿ïû›ûs©AGNbcu87GB 094609.3+583301?ïý6|uK?7NÞï?6LWÝ¢?7NÞï?ïýøýÕõ5?F+°Ý‰"ª?08PVOÁ?F+°Ý‰"¾?ï鑱¨D?dË]«Å ?fnNW»;?dË]«Åž?ïôï"/Â?E[AUì°?V Ù {ÿ™?E[AUìÒ4FGL J0950.2+0615¿à£FSÉ@EFA,ðúÀ:Zˆàä±ÆÀ<n;è
šó@ÐÉéC?ÿ`_¼(:?Á ¥¼è~.?ÀØÉÛ*Þ{@9}I׺g@«ÕÄF™¿ïÈ͙{f©?ïÿ3¶>ì¿â¢çUåã¿Þs²LîÆ¿áG§~´ì¿ïûÇVkF AGNbllGB6 J0950+0615?ïú5 of?Iat¯Hi]?G)~Bfo?Iat¯Hit?ïø¦‰¾Åª?bx¡ËH—ê?MeÙé[?bx¡ËH—ê?ïΖl[L¶?y—¹ë×l?x´ÉÒY¤Ò?y—¹ë×s?ïEjÏý$?…cË{µF?—R¦]»™?…cË{µF4FGL J0950.2+4553¿ïÒ*	@Hß`|A™þÀ:¸7êRÀ<…Q(ÀB@ŸTÄ}s?ÿz"¯tÍ1?¶-z¢§>?¯6¨¢e?ؓÓ›fù@<ȋ­?ê;KÀ¿n¿ÑÄÝÀ$5¿å4Ô#&¿Ò¶´DÁ¿â2«ž~Û¨¿áÊFà!AGNbll3FGL J0950.1+4554RX J0950.2+4553?ï塞ߓU?VçŸ*<×÷?`ZS l«ó?VçŸ*<×÷?ïûïSØþJ?Tà¼'iI?@B°œ×b?Tà¼'iIœ?ïáÝ/îò?q\ÝZ±ð½?n"ãÐ
•?q\ÝZ±ð»?ïÀ'Q:´?i»ÅØbª˜?¶ð×b¦L?i»ÅØbª™4FGL J0952.1+3932?ì–Çù;;u@I€Ž6FÀ;rð\À<Ø£oqY@!‰Œ{ÎØk?÷êÐ"¢§?Óå¿âÙ~Œ?ÌyÞýPù?ü5K÷OWV?ô ˆ­Ž¿ïÿÿ" 5•?ï÷‹Pb?í€ðÀÇÛ̿ӊi%¡_¿ÔÌåÄ—¿Ýx(Z½ëAGNbll1FGL J0952.2+3926RX J0952.2+3936?ïõÄS?T㣺…i"?TÅÂwYê?T㣺…i‹?ïÖëÍ®?N?')³£¯=?tŠ(àY"?')³£¯>?ïNÉ˟ˆ?'tÒ'Á¸‹?–&ƌÿo?'tÒ'Á¸?íH$K*?¢Ä¥§g …?µ¾ßM§f¼?¢Ä¥§g …4FGL J0952.2+7503¿àãÒhùP@BŽÌ¼Õ,À;}§´æÀ<÷;«§¹@#2Xëÿm?ò:¦ú«,i?ÜHñáYKÌ?Ô¶VÿIh@¤m'Lž@7mŒöH?ïOÄÞì´õ¿á¶2 ä|¿ï¡±`_¼(?î»4ßZÃñ¿ª]{íñ¿Ì‡Ú¿Ô–ÆAGNbllRBS 0804?ïöÇÚáH?Tƒ/Â,A?RpJ=o׍?Tƒ/Â,4?ïû^ð÷xY?X+;ÎYÈå?B"<"¡\?X+;ÎYÈè?ï¬èæMZ'?'YÆéM«ý?"ÅÆl©vR?'YÆéM¬?ïöKé\Ý ?PëÌ·[6Í?Sh-FD¿E?PëÌ·[6È4FGL J0952.6-5048?ïõTEëRã@9¡vݬïÀ:ªî!±*°À<2kÛñ,þ@ rUãâ=!?ÿD*Lä'?ÎۂGB‰½?ËÁЈgB?ýIƒ×u.@	qÁpÎ\¿ï'Óa'jv?ïøx·¡Â]¿ÔìKî¿ØCe'Š,¿éý7%?¿È¡ð•©ÊêAGNbcuPMN J0952-5049?ïùn`šH?P¯Ú&"?JF}—²ß?P¯Ú&3?ïÏÓ|Åí–?˜ ¡È'÷e?xA	4ä?˜ ¡È'÷e?î'?òßÄþ?™È•—"É?§ÜÒ°?™È•—"Æ?ïÆÅè÷I›?o°ý=´?|"[2o?o°ý=´4FGL J0952.8+0712¿íÖÒ('˜¯@E£?á—_-À:ñùÌàÀ<¢Jmâ[ª@ IúõÕ?þHåL"C?Ê¿Yòª?Ïã}h`'@]ˆ~¿"À@Ën–™	¿ìø0Èõ§·?ïõ>¦-ü"¿Ø"GNNí¿ÔžÒn¥Ð¿ïþa?ïæf¿QºAGNbll3FGL J0952.8+0711SDSS J095249.57+071329.9?ï›97v¾Ÿ?—\|²r^f?‰1²"PWõ?—\|²r^e?ïÊZÒÅë?"ÉN^Üü?zÀR–
Ó?"ÉN^Üü?í€7Ã?£q³k~
>?·+þGyç‹?£q³k~
>?íç>õ±é?¡Š]½@â'?°ÆWp¹?¡Š]½@â'4FGL J0953.0-0840?ڡتzˆÕ@@óO?Ù3ãÀ8d.˜™¿YÀ;n­£;ÙË@ßn"³*å?üכ'˜™?£Ú!þNò?§Ë
te@ždoa'@
v4‹¢àë¿ÊæW¸M¹Ç¿Ü{±|9av¿Úä1ò¿Üžt?¿Û#'K¯¿ãO"þ)f+AGNbll3FGL J0953.0-0839PMN J0953-0840?ïüæÈ­å?2ðHE?8É¿'Ýê?2ðHk?ïú¼oËj?]úõyž?E@ÒTD?]úõyŸ?ïÖӊ¹Ùr?zµ½û?t–:£FÕ?zµ½ÿ?ïæó¨Ý
K?RÊõ¯
ð?iW"ò³Ò?RÊõ¯
æ4FGL J0953.4-7659¿Ô©+{­'ÒÀ1Š©Å`ÇÁÀ:½c€ßÀ<`wç˜*.@ ø£8bG?þ¯(¬ÇsÇ?ÎÙh¼ûî?¡·×GO÷?Ñí_‹Íÿ?üY˜Ý±÷^?îz	{©ÄŠ¿æ³"µ!¿ãÞÞyÈn¿É@٘b7¿ãûD^Ô¡­¿ÇZ<!~|AGNbcu3FGL J0953.1-7657cRX J0953.1-7657?ïþrK?'ÜtûX˜?(ÛOþ?R?'ÜtûX˜½?ï÷"gçó?cЄƵýÐ?P÷1Ä0­?cЄƵýÙ?ïöž­`¬?O/ahľ?RÂ¥?Ô§?O/ahđ?ï¥Z¾Ò~?oÂÛA?†©K`9?oÂÛA"4FGL J0954.2+4913¿Û7SÒ@Hɛ^•·À:¸®.|NÀ<iU1Š¼‡@!¼'?ò"EW"%Å?Ë*D¢s?ÔÍ¿Ü#å@
)
]Qï?þ%2êc
¼¿ïêzAå}ž?ïý³^f¾¿ÙÊɝ}u?ÒóbÎ+qž¿ÛV¿\W¿ÐtéæAGNbll3FGL J0954.2+49131ES 0950+495?î4QB"»?«¯ÿ
·å?¬ºë×&ÄF?«¯ÿ
·å?éCú?§j7e\Y?‰ů<A‡?§j7e\Y?ì$Ûš¤?«|½G"Á?¾Ù'ß*æ?«|½G"Â?í4¸t? ð"´ž¸¬?³—VZ?œ`? ð"´ž¸«4FGL J0954.2-2520¿ääMÕqG@6_Až0PÀ:¢Iøq–EÀ<~ÑF¯ú@ /
Å"?ÿ‡šÉD'?ÄqÁ¹H`—?˜Žd.d?ØÁ—¯@÷
ú¯ß?ïÿ!ڛB¿Ür½'ÈF¿çp4摙ñ¿ÄP'à™³E¿áHÍcˁs¿ä'gÁZRÝAGNbcu2MASS J09541965-2519588?ïü-~xJý?:™^ ©±@?>"=¨·?:™^ ©±T?ïýp²<?QP">ÁEm?7ŒzoR?QP">ÁEa?ïë{.¸éæ?iq#"L1u?d"ÑGÃ?iq#"L1T?ïԔí•fá?`1
¸][¦?uµ‰5L"?`1
¸][°4FGL J0955.1+3551?ïüãŽ.&M@Iß°_®¼AÀ; ˆÂ±ÀØÀ<ôæ¾æZ=@ œ"†Z"?þ$àŠó?ȦˆÂÔ?™µ÷ü®ðL?Ô|Š_iòã?ü¼xÁ²½?ïüÿ?:Óf?Òß<ã[/¿à¢»ìª¸¦¿à. ÿÿÕ
¿áÃ_eÁ$ù¿×m\D#›fAGNbll1RXS J095508.2+355054?ïü¦çIê¿?J$(*Ñ?:ÈÅ°ª}?J$(*Ð÷?ïøÑ£aj²?b±r¤Œ7=?L¹rzU5Ô?b±r¤Œ7B?ïתòíq:?{1U~£èˆ?t*†‰GbÎ?{1U~£è'?ï…ÓBp!?w''nŽô?Ž‹;oc÷"?w''nŽó4FGL J0955.2+0835¿äÑÔX"È,@F=ã!¢ç÷À;Fiž)KSÀ<™§ågÎ@D‡Åܙ@ø¢×/ý?Õ@'&5t?³Ä»[`Mó?Û£VœCíì@4§®/RÔ¿ç=:¾Aê|+"Ù@y¿ç0iTWp)¿Ò¦^äfòR¿æuÌ}ɯ¿ïò›]¾÷øAGNbllNVSS J095501+083342?ïû»»è?A«u阻?C‰°^"?A«ué˜Ì?ïüd?bR`¹ú}?<Üïßp/?bR`¹ú…?ïÕ#0,»?xŒ7©ÜÍ?ungé¢q©?xŒ7©ÜÊ?ïòÖbôô?JÀÏfŸ1?ZS:âš?JÀÏfŸ14FGL J0956.0+3936?îÿÿÆÏ»K@IÞ<âž4À:ñù²%hÀ<½>Õ'å@`ÕwuW@Ò7y…?Å
½]Äu?ªéLŠGA2?á…Ñqw<?ý"È<V?î™Ä%^¿Ö‹_ú¼t:¿èŸœb¡µÈ¿ãV:Ÿ8?¿áBUå墇¿ïÿú Âî'AGNfsrqWISE J095608.57+393515.8?ïðúøЮÆ?Yït奸f?^
^¢s¨?Yït奸v?ïÓì)*"?Š!-z-e?v	ëj½û?Š!-z-e?ï}v?‡Ê\\փ
?Q?\ü¾?‡Ê\\փ?ïùÇ9Â^?‰Æ†£IÑ:?Ÿ ÇÇ´‡?‰Æ†£IÑ<4FGL J0956.5-0958¿ï«.E‹
@@ÖÌ¢Ûa»À;‡þzÄÂ<À<¿Ã€ó°f@!ªpI¿Í?õ^x%«‹4?ÞH×à&?Ød¡ŸøXl?úª(Èv%÷@Æ+rõk¿ïúŒ"¸'¬?ïÙû¿(Ÿ[¿çã4å2t¿½‡âž+ŠÙ¿ÜNczΨD¿È§^hÁ	 AGNbll1RXS J095627.2-095720?ïùI¯"jì?EœfÆÄàŒ?JÙCvTRŸ?EœfÆÄà?ïû™^5sh?]ҘvNª>?Aš‡*2d?]ҘvNªE?ïµe+3¹?'©ê­ «?'¦µ?sÎ?'©ê­ ¨?ïã¶CjÊÑ?b׿4÷?lI¼•5.E?b׿4ü4FGL J0956.7+2516¿ÓÖцŸÛª@IzÒ4ëšÀ9FÁ*ØßÀ<Fx*´±@zŸÉ3%@ç	#•0~?­PLž"*?¸cÐ^ý'f@~5Å´ª—@0ïŒv¿Ðû"‰µ ¿ä¤
ájÿçb)Àê¿èû¶ßû}º¿í¼{Eñ¿ïúàSG%AGNfsrq3FGL J0956.6+2515OK 290?ïýô;Õ
x?*4o(<"?0^!W"Kš?*4o(<l?ïùÂK?í?b©Px¿÷R?HöÓKÊD?b©Px¿÷Q?ïÄ+ÅH)V?y:ÓùD…?}ê[ëTå?y:ÓùD…?ï㡆À¨?Yäà
×s7?l^yç?X]?Yäà
×s54FGL J0957.3-1348?ïq¨ºÖÞ2@?.+{®ÍÀ9¦©ÑAåÀ<*ø; ‡@SŽºB†@zÕٻș?¶r ®Ì1?Ãà:±@0
ÚN•@úÓ>«âG¿Ëƒw™?¿á†"S¼ì¿äŽ4 C€¿èqéòwA¿í$ŒVºø¿ï髕D CAGNfsrq3FGL J0957.5-1351PMN J0957-1350?ïöee~üA?PñYܙšÒ?S555?PñYܙšÏ?ïúÁ0?f¬ìÐY?Ä?Dû¿¯=Ã&?f¬ìÐY?Ç?îÝðHgoÒ?™sWæi;?¢ ûy‰å?™sWæi;?ïô•'*½þ?BØ€^?VÔûª"þ?BØ€^(4FGL J0957.6+5523?¬‡Ykò¶'@G÷7âÅ\–À7Ìo¯»DÀ;+Šƒ|!@º	^" ?þgbzH›z?ŠñnÝ`÷?´
š7Ï$@@%Áã†Lµ»@
%@톿±ªà=íÌL¿ØběOý¿à•OB2"¿à[
bY'l¿äS¡2OB¿åTWp)]ÇAGNfsrq3FGL J0957.6+55234C +55.17?íÇ$Èd7?°¤~äא?±ÆÙ¿tÞP?°¤~äא?Ñ%¦ØV)?Ùµýà?çm,ö"Ôì?Ùµýà?í@Å÷â`?¦õ½@.¤½?µùÐCìù?¦õ½@.¤¾?ˆx¢¸Õ?€Jp4¡?–u?€Jp4¡4FGL J0957.8+3423¿ç»£…¼Fù@J&îcŠ	À:t¥×ÛÀ<®!õô
ƒ@)ÒÉ*@q<%J<d?À–%›Åî·?ĸØú¹>@(C(†@Ž e¨"?ïû›¢|K¿ÜqÎäÕO¿ábTŽ†@¿âWÝ6§[ú¿ç¾RúÉ¿ïöCôK–×AGNbcuB2 0954+34?ïî0WÍ?l¯¬É?aæÏä¨38?l¯¬È?ïûl6÷ç!?U:ْßü?BO$ c|N?U:ْßù?ïyèÁ~¿þ?Š?üQà÷?ÂçÐ(S?Š?üQàú?ᅬ²ƒdj?eƒ•l̯ÿ?€_&åe?eƒ•l̯÷4FGL J0958.0+4728?íþÉLX›@IU·|¯ÞÀ9›"²ÈÀ<1Ø2[@¿B4Íg@ì&ÿ½?²SõuuÊ?Ð?½t•@ge47?1@ùnõG¤?Ìÿ‡	I)ë¿Þ²…³¹€¿éTÀ¡›EÁ¿ç‡»JÄIq¿îíŒàΌk¿ïÿ "_õAGNfsrq3FGL J0957.4+4728OK 492?ï½K`¨?—÷VØd)z?È\¶"êí?—÷VØd){?ïót'äÉ3?võu¿¢¼?Yú6m™+?võu¿¢»?ëÜÀØAŠœ?¨s-Fž+Z?ÀŒüžùՖ?¨s-Fž+Z?ï¨iê?PÍþ÷Ïìc?ab\W–Ñ?PÍþ÷ÏìY4FGL J0958.0-0319¿ïOÛγ†@C%? §?À;œ¥ŸaY·À<Ê]Óð­}@"˜ÕV‰#«?à•<<Ç0¬?ï6jXŠÜ?é±e¾àÆ?üõÅêZ|@²Òû¿ïýcm¢?eÆ-¿ÖUGZ1¥¿í€ãŸø†?ê·ãÑ̿⨈ŸÌ8¨AGNbll3FGL J0958.3-03181RXS J095806.4-031729?ï£ë%P{ê?­âbÃz?‡6«á¤?­âbÃz?ïý!\Á;#?P"LÛÉÎ?6õö&çB?P"LÛÉÈ?íÙÂS÷ûz? o*bbÎP?±1í`@$)? o*bbÎP?ïúɤ«+u?LªõÙ¤?DÙmSR$¡?LªõÙ£ö4FGL J0958.0+3222?ëyY61í@J!æî·`À:oÎ=UÀ<A©î{s@{k™¬@Ý«ýIl[?¼u_þmXÉ?°ç1ýÔÉ?ðmjœV|@"ëa¸W?í™j4Q@d¿ç@6¡|¼ê¿çE\á,€<¿æLs@i|›¿ë—¬ÂkJ¿ïõ´¢‰'JAGNfsrq3C 232?ïÁÎ×.µ0?…‡°('{µ?"h¥gÛ?…‡°('{´?ï¼3;A ?"Ö54É£?€ó1/¾ü?"Ö54É¢?ïƒ`ê»?†¤ýp¹?'ûÅ~'I?†¤ýp³?î¹d¹‡˜?'"
 ÁFµ?¤i´g†~e?'"
 ÁFµ4FGL J0958.1-6753?Ѕîw
ñ•À$™ë…¸RÀ:ö•mºîÀ<C¾˜V£{@始ʣþ@ùPá™ãk?¿Yô›¿´B¾$=w?÷­N·ó÷´@Y±rµÕ?Ԓ{'­Cð¿ä¿ð{'¾‹¿èH4rß¿áŸÿ¿"SY¿å´ÊAؤ?œñ(™À'AGNbcu3FGL J0958.4-67521RXS J095812.8-675241?ïøOÑ?d—?VÏ6Ǚ›?NÀ»m¥Ÿ?VÏ6Ǚ™?ïúq4áB?awDŸ?F;-ˆzõÎ?awD¤?ïèS@Ð?uËáÕ¬çæ?g¬p¿o/'?uËáÕ¬çá?ïÚÒ4µ?a‹ÿ2(*,?r–õq奠?a‹ÿ2(*(4FGL J0958.3-2656¿à˜›±Q9÷@5Éó×ӑÀ;EeÄ÷1À<ª%s@-ÑRB˜?ÿùI²Ñy?Óû¥ˆ€?ÎrW`dÙ?üX(&·@õ^'?¦ÏF_ñéM¿Æƒ¨9¶°¿ÑߥA˜{·¿ßƒÄKžå¿æ8ßå®E"¿ïý²èõø?AGNrdgNGC 3078?ï€~ô7ß©?$^Š0{?àBòT?$^Š0|?ïåJ.f½Q?'Xâå†~Y?jµÑ™B®"?'Xâå†~Y?îëü²"¯?"Mp"^?¡@4×µ¯?"Mp"\?î«ÏÂáûµ?†–X€WÇ?¥CÑàD£?†–X€WÆ4FGL J0958.4+5042¿Ë_Ëò> @HâãK"SÀ:bŸ1‰À<²Š¬–Ì`@iÂp}k'@ûµ¤at?¾ª ¹.Æ?­s\f³=?ê×'[å@
ڧ옚?â<x¡|g¿äÿïÕ¿ço˜p"¿èàíìEz¿ëèߥ¥¿ðAGNfsrq7C 0955+5054?ïýóӋÿ*?-bõ~ÏVÛ?0ac ´æ?-bõ~ÏW?ïüŸh¢œ?RF·?;ºïœ?RF¿?ïça>].,?pôùGjúØ?hžÁ¢ÑÕH?pôùGjú×?ïæô"|¿?WßÎ*'ÏÖ?iákƒA?WßÎ*'ÏÉ4FGL J0958.4-2441¿êè
yU|@7|#̍ãÀ:rçy }NÀ<WË/=Û-@º+Kˆ?@	`Z³«?Áw÷ˆàd?É øžï"@È9À.e@)Ï/þuf?ÓÏ6JÀ¿ÛQc'A¸¿ÞÓA:ÝÌy¿âQ(Fp&Ú¿çñðÃL¿ðAGNbcu3FGL J0958.6-2447TXS 0956-244?îå¨ÂÖ?¬OJž2$?¯Ñ¥sҟ?¬OJž2$?ïÌP8MÎ?¢‡N
=>"?yö×ãÙë?¢‡N
=>ƒ?ì´>5—?î?«\ÑØÃ?º^SF?«\ÑØÄ?îxNMQ"?ˆ°Z"O?¨~[*íë?ˆ°Z"O4FGL J0958.7+6534?ÕAlÓÏ@EYtæ[êÀ8rÐ4³À;´~d‰íT@êƒ-±@Kv Í|?"åL"C>?¢ÿPËN@BåۑŒ@¦±['1É¿·(ÃÂ>~¿àåÜhKBô¿ãƒÿiKZ¿âýò^¬³¨¿æz¿^z3οᘼúDZÛAGNBLL3FGL J0958.6+6534S4 0954+65?ïüöN_íš?5kƒÆGþ?8M"("?5kƒÆH?ïû!Á£†?XºˆÍ¥³?C{üùqèä?XºˆÍ¥³?ï×™TÐ?wbd+Ë/?ts3U—ôØ?wbd+Ë.?ïÿû7Ètõ>½®=SÖ>à Þ,,O´>½®=z¢4FGL J0958.8+7039¿×ÄC¸©hã@D$ p¹À;Çp‹ÔÀ=%Æc&@@!í³/³ø?øÿ&¡Txþ?×ÚQðœ5?Ñ${tëdh?÷ ªêúµ=@ߘ¬^ÿѪN½Ó4Æ?Ö{4©«?áÝhã³?³àΌj‡¿çP䉁ôa¿Ì.îúâ	AGNbcuGB6 J0958+7039?ïç¦Vðu¼?cx¢*aÎ?hY©ŠDÿ?cx¢*aÒ?ïûÇ»`ñ?`©
¢Å¬?@á}È<K?`©
¢Å¬?ï¥Ï}IQ?"eãa37p?†Œ ­«¼?"eãa37p?ï®É-ÃÓ?r7p¤±?"M´9ŠÐ?r7p¤²4FGL J0959.4+2120¿Ô`¶ 9Uñ@IH8Ÿƒ¾fÀ:§]u&ÊÀ<…='[·@€Ù% £y@"NCYñä?Àªa½à濋—/Üçw?Éü»§áZù@gNåúÆ¿ˆ@ïÎs¿ßpš1o
Õ¿áéžÊ[…¿ãgS–€	¦¿ß†3‹GÇ?¿á¹ASAGNbll3FGL J0959.7+2124RX J0959.4+2123?ïðø«¢Èø?Ww™k•?^¨ºn­?Ww™k?ïý_ :ñ?M87̹'?5þ(u¸?M87̹ ?ïãu'ò´i?s'§iPÏ?lŠØ
K— ?s'§iPÖ?ïñæÊL'p?Gè€ä$´¯?\2kfû ?Gè€ä$´¼4FGL J0959.6+4606¿æ­VQ7Š@I¤¹#¢œxÀ:¾=¢ø½ìÀ<u¾{Ñ1¶@$›7(‹:@Róš–ï›?Â×ø…bU¿¤E_@éep?ÚµgÀÙyƒ@=Ò™™?Ú/é(M&¿á­ïýS}V¿ê^ç$.³¿èP"Xð\¿ïÿòÿf}
?ïr·bWcAGNbcu2MASX J09591976+4603515?ïå%Àº-×?tN¶A_Te?jÚ?EÒ)?tN¶A_Te?ïQoÿ¿ûÂ?°ìãLJ–?•Ò‡Õ?°ìãLJ–?ïl1G"~?‰™¥l&h8?'y×
?Þ?‰™¥l&h9?ïafJç?ˆXKiEE?"Ó6£ބ?ˆXKiED4FGL J1001.1+2911?›ËjÕGĎ@JOKrÅzÀ9z¿ª¥Z˜À<^×,¢z@wÐ1[AÅ@ä#¾K)Ê?«ÉªƒvÂ?®éO[Õ5I?þ¬5}N—@kd°-Û?ÁZê‡GÝd¿áÜ,¼ ­¿ä¾ýÝ;¿äÍi_•ô¿ã˜†t"è¿ß¹ö{œÙjAGNbll3FGL J1001.0+2913GB6 J1001+2911?ïý}õ@ì?0'ÛÒ"'Ü?4Uÿ§·?0'ÛÒ"'ð?ïü"vÞ¿'?QÚÕÍÔâš?;\I
È°?QÚÕÍÔâ›?ïëkšoó?hIŸ\Ínï?dr"e2?hIŸ\Ínâ?ïÿŽÍã¸>üô}¶Ëˆõ?L‡9	™>üô}¶Ëˆó4FGL J1002.5+2215¿ïwð#Ðâ@IÂ/¾3¬ÖÀ:Œ¬nˆs×À<wXï…^y@ žv{‡_Û?ýä(3$ðz?Å‹ypYY?›˜+§Åù–?،üÓ$Õ¢?ðÆ+«T'
¿Úם‡ý¿è
ÀGƒLP¿ä.]
¿Ô"ãQs¿áƒ÷ÜEÕ¿ÕÝÖÿžAGNbll3FGL J1002.3+22201RXS J100235.8+221609?ïüQÍ5öÜ?=FÊ4)ô?=q–PIŠ?=FÊ4)÷?ï£f¶ÄÙ?žoõà¼0ý?‡?æRNÉ¡?žoõà¼0ü?ï鎬uW'?oÎpÒÎ?fqSŠ¨p>?oÎpÒÕ?í¾°1{¾Ü?›dšÒq[!?²
~t"	?›dšÒq[ 4FGL J1002.8+2140¿Ûï›ôו@I³ÌcñA À;c$W@YÀ<ÂWþė@ÖZÖæ+C@˜ûyˆ'?ÊôµÉû⿦³vºq€v?Ùy3]$žE@‹ž†é=ǿ什ÿT‰o?îE¶Ãvö¿é=1ïfTÉ¿ÒUUM9¿ïªøÎÞ?åo‡wX&2AGNbcuNVSS J100250+214225?ïÐÀŠ‡•
?|½dks¢`?wŸº¼5y?|½dks¢b?ïû¢w?cït$.‹»?Awç·ª'É?cït$.‹·?ïUœÜH%
?Ž¾Þóo_?•Ldvû^v?Ž¾Þóo_?ïïºÿNj?Tu©°ÜgÆ?`Eþ8t?Tu©°Üg»4FGL J1003.4+0205?Õâhm*˜(@ESøüÖÔÀ;9|"NÀ<¬#þ	ù@Óy³J?ÿpŽ•·?È´ E°8m?°Ü_çÇ$?å•ò`L–?ÿµ³–??ïî"%âؿꐀýÁ?³$œ—zÛh¿è¢JBCqo¿Ú¹#ã	$A¿‡.tɉ)AGNbcuSDSS J100326.63+020455.6?ïýcŒËîÙ?-£§€
«?4㙠‰;?-£§€
ô?ïûûy‡ÙA?Zsí_¸X¥?@àšû?Zsí_¸X©?ïßdíª?pØd"¯¦?pM‰*ñp?pØd"¯ž?ï¼ÀÀÒǘ?n¿f®Ï˜¤?€ÏÏËNö?n¿f®Ï˜¢4FGL J1003.6-2137?Ð-4ÐÛ;@:ÐEþÀ;ŒŽ·¾HÀ<À
(ÝnÛ@"ÿ2ûé?ùú5 Ë½?Õ¦_»&‡(?ÀJ
MzÝ?ëbC¡ÀY¢@#fón¢¿éaßî聿é/"þ)f+?ï:Î2'šy¿Ø7±G5H·¿Ø5H Öj¿×A¼ã˖íAGNbcu1RXS J100342.0-213752?ïÿA»_fq?öÖ¨÷ ?Ȕ2"Ù?öÖ¨÷"?ïþF@‹Ú?@¥"×Åà­?'›÷B\:?@¥"×Åà«?ïöÿžõI`?XÉg®wÝa?RÂm@c?XÉg®wÝD?ïúáõâ
–?4µ"¹!ø?Dx(wɨ?4µ"¹!«4FGL J1003.6+2605¿ìMd÷ö4@JTX`fÀ:›k¯{ƒ.À<wú ø@
?h ¨W@"¿'a?Äð!e«U"?Â3£Æn8î?÷O­¢e6?þš<â(¿ë{L§xn¿Ù2ñ#Ä*g¿ãrZ?çvœ¿ç[§J¿àÑ۔æ¬r¿ïüfM;òõAGNbll3FGL J1003.6+2608PKS 1000+26?ﴇ'óï+?'%sm@€?'Þ65<?'%sm@€?ïÝOã¾Ë>?ŠCœ®:ô?qX ša}?ŠCœ®:ô?ï\B3%'?Œ)¹Ü‹¥?"w¹›M¿<?Œ)¹Ü‹¥
?îAé cÚÇ?™Ò´µÀŸ?«ámùÂSŒ?™Ò´µÀŸ4FGL J1006.5+6440¿¨Á°ôìG…@F&¯%;À;*.XØß*À<ç3cښì@ ÷êÃز^@©}'Ô?ºrzù*¤¿¿Õ€r'?òXåªda?ÿã­¹â}¿íÐQò;_¿á½c£=‡¿â\ᢜ́¿ÖGKCdt¿ä	Úÿë]1¿²zs8±ÍBAGNbllRX J1006.1+6440?ïù5/‡?AÝ*ÒÜ¿?K+ƒ"Aæ7?AÝ*ÒÜ¿?ïö²£¸_?s¾\ÇŸ3?Rš¹öCö?s¾\ÇŸ5?ïìß݌7œ?q8ϐ/¿Ï?c "sÈe
?q8ϐ/¿Æ?ïŸÅÀdea?uƒ£h Ôó?ˆææ§o?uƒ£h Ôö4FGL J1006.7-2159¿â›6®Žj@:Æm½r¼¶À8aKŸŠÀ;ÊÊ·H×	@ê'1È$@ZaÎQ1?±!ð@+?§Œ%'¶¦p@хÞz@¿´Û>˜¿ÂŠºX«è§¿â}Wyc™-¿æ8"œ×%¿äÙ>ö
¿äìÉA|÷ø¿èw]š
_AGNfsrq3FGL J1006.7-2159PKS 1004-217?ïýt;Cs?1I¸Š?4_~%än•?1I¸¯?ïû¤ðpÛù?fhÀÑ%©<?Al><¥?fhÀÑ%©=?ïÕy™]ß6?v»5 ùÖ;?uC3Qe2?v»5 ùÖ0?ïÿü\s‰>¹{"s™	>¿ÅcºÁç>¹{"s¿34FGL J1007.0+3455?£Ïò: yš@Kà?pÀ:š¯_Ô{îÀ<Š®¬Ÿ0@ oè;=B×?úùcc|§?Ã#öiÔ/?Á*¢jùs@Òz{Ç!@g&q÷?ïÕřҤ}¿â†ôæÇIÖ¿ËåÛf˜Z¿Ôñ§ãxu¿à ÇuË¿ÞE`Ý:ƒAGNbll3FGL J1006.7+3453EXO 1004.0+3509?ïðOgÐý…?Xžd4…Œo?_a0^öG?Xžd4…Œi?ï÷¿;×_ä?d.ëÆwÙ?PˆQ@< ?d.ëÆw×?ïÝ`@x?røâ|[$´?qpÏßÃùœ?røâ|[$¶?ï"gßrŽ? ´M+?œ;³®X? ´M)4FGL J1007.6-3332¿å
"vî+@1õßeUÅÀ92 
¼À;ûN']Šö@¶‹¤ô@<ï>çœ\?­ý"ÀÁќ?Éü§ZøI'@ÿõbLM@÷Æ0{s?Юý®ìè¿ÞÁ {öpŠ¿ær¡Þ¹¿èkˆVÚØ¿éÄP'èË0¿ïÿÀtϵµAGNfsrq3FGL J1007.4-3334PKS 1005-333?îÓÏñèÄ? †}¦Jæ?¢ÃáÃÎ? †}¦Jæ?ïàÓñ¤Ç?Œlº.¢¹?o,[8öÔ?Œlº.¢¶?ìS21©?©²®kÅ?¿ÅfnrÄ?©²®kÅ?ïè¸ca?TÚpgéȀ?gGœžïäÎ?TÚpgéȂ4FGL J1008.0+0620?ß,˜úÓEV@G×süÀ9*¼ª?ÚÀ<¼ bv@Ù'ÌLÊ3@B+{®Í?«0ªþ×ó?¨)Ûúë?ü´d¬R@ºË…$?ïþ[à¦sr¿ÎBßN"¿ãíÔï°ýc¿ãˆ¿V"¿àºÇ犾5¿èZ€êv+AGNbll3FGL J1007.9+0621MG1 J100800+0621?ïýö™¬w	?*ŽpÎ?vy?0K2œGĒ?*ŽpÎ?v€?ïü¶…+ÇÏ?RõY"?:KÖ¡Á…Û?RõY")?ïÌåÖá´¨?|48ۃêC?y%¬?|48ۃê??ïøapY
 ?;'—Í•ÂÍ?Nz>›×z?;'—Í•Ã4FGL J1008.0+0028?¹L	C, â@EO'j@À:O{ûùáÀ<n,·/¢@1¡&@&býüÁ?Ì-µÅÊ$?»¢""EA©?÷'!A™'"@Y ­ ?ïÿü¥¬¨¿à"ßq?¿â&±$ÿà4ÚÓÍ%¿êø×ý­j\¿ïÿ‰XAGNbcu3FGL J1007.8+0026PKS 1005+007?ïïÌ+°3d?`	A'šÕº?`3ÔO̜â?`	A'šÕ¸?ïðŒØ?c7?q¨Çq‰.7?^æO9""?q¨Çq‰.5?ï²N+?";$Ýò'‡?I¶=z:?";$Ýò'‡?ësñ?‰Ñ°¿ÙÊ?¥4ñHÀîÛ?‰Ñ°¿ÙÌ4FGL J1008.1+4706?ïÁœ`·ì@J4ÿëJwÀ<	zP(6€À=!iθ@"tRBÂó/?ÕÑȽ/v?ãj@ºˆ'?ï
{é…j@1¤Òh@|<yX¦?ît#=qÐ}¿ïÿúÁҝÇ?ïÿÒ†ëA¿Ü9™aܔ?Çaû'©¿é- qäAGNbllRX J1008.1+4705?ïópÒ®õ?aÜã³·È?Y[梟?aÜã³·È?ïúÀ‰q>?]ŽÅI˜T¢?DýÚ;÷;?]ŽÅI˜T«?ïYŽý?þ÷¤îÇO?"ÝÎ><K?þ÷¤îÇN?ïöf=ÐP?VW1ê,""?S3"_Û`-?VW1ê,"4FGL J1008.7-2909?Ð9¿ì@5ŽÊW§†ÂÀ:Œ½½eP½À<ZTtÌZ·@qgd"(@ic¦˜…?È
£‡"S?̦C̪ï@€†
 z@
Wr,Ã,?ïÿÄ}îB¿å«fJ¸¿æ'F–½FG¿ä‡`F'´É¿ïý.>Åè¿îŠøìæGÈAGNbcu3FGL J1008.9-2910PMN J1008-2912?ïݎ¨
<?tøä–¢ž?q8«ùáé?tøä–¢?ï·Äétw?¡ù'(5¼?x¼‹EÅ(?¡ù'(5»?îfà]ŒT'?˜åè}i?©'ú':½¯?˜åè}m?ï(3??)O§3°?šÿŸù ??)O§3±4FGL J1008.8-3139¿ï"ÿ	ÛQ@3˜>BZîcÀ:ç6žËÀ<•ohm¨@.tûª…Ð@^ܙÉjB?¹ÝâHßí¼?¦/³Ýù¬?íF¤>¹#M@Tóe轿âÖ÷ÞshX¿ä>Sü×W¿ã/c?•l8¿åú,hJl¿àlk΅3±¿êº¯"ÖáúAGNbll3FGL J1009.0-3137PKS 1006-313?ïÑ I¡ó?rÂÐ@L??w/ô[/l?rÂÐ@LB?ïùº¤­e[?b㙏A"¶?ImJj'€?b㙏A"¹?ï!ØÍL?‡a0䈽?ˆ·‰Ì¬ÿ*?‡a0䈾?ïĘ9«â?k|äZóÕG?}³ãq*™?k|äZóÕC4FGL J1010.2-3119¿ï²(ºÝ@4äy'¼À9"pæòèÀÀ;úio/bÄ@!PC÷¦•+?ûã#·;k?²'rásøË?'ÒóYçl?â3òí†+@
!"}ö¥ä?ÁrI«7?²L'S$¿åŠÛá<ÆZ¿®æ¤ o¿ä¦],+6¿Àf‹û r;AGNbll3FGL J1010.2-31201RXS J101015.9-311909?ïýŠ)'çÆ?+±>üöÏ/?3®³pÁÕ{?+±>üöÏ<?ïûÖ]"H"?`þ×H A
?@¦‰®Ý¯d?`þ×H A?ïéÔåt¼›?q
ª]n`5?f+‹Ceu?q
ª]n`+?ïú)'ÀL?<ìäâè­õ?G[ñ´þÖî?<ìäâè®
4FGL J1010.8-0158¿³ú'^o_J@DÍæÿ}úÀ:$<ù…'À<UäíU@q"–ØÊ@gÅá÷?»ÌBŽDü´?§M༠ŠÃ?è®~F¬ã@	–­…èÝ?îþê÷Z?¿æxK5ˆx	¿æ'bO*‹¿ãqYßofÀ¿ïýé:ø$¿ï4v"±ÓLAGNfsrq3FGL J1010.8-0158PKS 1008-01?ïöéQ"_?P2©Í?x5?R-\ÙAúŸ?P2©Í?x)?ïûð¤6P?UYgÊÞ-E?@=o&¿¾?UYgÊÞ-A?ïã‡8—Ù™?mŸ)%™¼?lxÇh&g[?mŸ)%™Ê?ïÌÇ[L?g¡Úìu?yœqRzZ?g¡Úìs4FGL J1011.3-0427?âôî´¦kS@D
êÈ`V'À;R%fÁÖÀ<y_×Öì
@£òž­œ@Òÿ#a.?Õ&¯aû?ÓFÚÕùò?ü¶¡|¼ê@
™«Ã<Ö¿×w؞è
¿å9£ûkq¿æ€Éë£R¿åo쌅´à¿ïýÕ{Zi¿éÏ
í6ÐAGNfsrqPKS B1008-041?ï÷EF†WÒ?W¼õi:E?QuróPZ5?W¼õi::?ïûð]{}?]«ç™ðª#?@>‹î€?]«ç™ðª ?ïWÀJ:¸?‰¼3¡{é!?•§ö¸¨þ?‰¼3¡{é#?ïâàF£ÔÐ?YjPqj?m¹\+/4?YjPql4FGL J1011.6+3600?íL*Rë*ö@KŠ($xÀ;%t…
À<Ú\ђ.k@)©m¢ñ@"õÞ>Y?Ë|¢¨a­?ÍwY}ʱ@A@š$?÷KêlQ¸¿ßC\¡¹Ñ?ïȯÑêBÿ¿ßG.<ÔF¿¿ç™mYŸ®‡¿áó:u¿ïþ®üØ-SAGNbllNVSS J101147+360019?ïSk/Fq?•Î°öˆ`?•'š<qÆ?•Î°öˆ`?ì\r‰}bz?Å&Û
¥õ?½k´ì5?Å&Û
¥õ?ìú°Œe?¦«'«MçS?¸/JCœÙ?¦«'«MçV?äCü‡îG›?·†íè6?×xð#pÊ?·†íè64FGL J1012.3-1232¿ãâ¦u;|@ARÒ^Ý)À:Ž-–;@HÀ<Rv'=\'@̀½)Áš@l dŽõÒ?Àƒ­Éý9§¿¢ûä"ºü&?á Ÿiè&@˜&+ô¿"Ów¤É›¿éÓïk]F,¿çç	Ĥà¿æ¿¸èz0¿æ›}Ëú¿®04âF÷AGNbcuPKS B1009-123?ïáÜÞü]ô?oAVЩN.?n#!¢ô?oAVЩN2?ïõ	ñP¨}?t)þ­ÄLû?Uì^¯O?t)þ­ÄLú?ï–'a ?ƒtÊÂy?ŠgºXF?ƒtÊÂ|?ïÛvsZ/¥?`ò*Ø 
Æ?rDÆRè-s?`ò*Ø 
Æ4FGL J1012.3+0629¿ÃØT…_@G~´À9v¹Ù«À;Ù;,ü¸M@ú£è'M?ÿ"~b®–?²äv6¾/?·åøÂÉé™@ëíœP-?@fŠŒ¶\H¿àÙCӔ¿ãsˆÃˆ€m¿Þæ×¥mã2¿á!‰¢«'¿áò] D-¬¿éçšät«AGNbll3FGL J1012.2+0631NRAO 350?ïúÌÃó?@Ø
3»\v?DÌð3óì"?@Ø
3»\ƒ?ïøÒæš?]Ä©|ÔWê?L·ðg'™?]Ä©|ÔWê?ï׍%@Ç¿?v²ÝN?t9m_œ v?v²ÝF?ï'2tΕ£?qëÔ¶X?‹sbÌZ—W?qëÔ¶X4FGL J1012.7+4228?ᝒw}Â@K4ohÜÀ:hÙÒnÍ=À<v½ôµ@ Žòµ¿•?ükWfï"?Àš<VÈ? A>â?á/WK@鄈»Oø?ïä]ý⎿æܬ1&é¿àö>"þ¿Ì¨µUⵗ¿áÍ)HÎ¥ë¿ØüŸxUÒAGNagn3FGL J1012.7+4229B3 1009+427?ïÿEŠw³ó?…]š«@ž?N±	wy?…]š«?Ø?ïý9j
?MidΤ	 ?34¯_'L?MidΤ	6?ïûŸdâ?UåŽÇ'9?A'oÄqt?UåŽÇ'c?ïò¤C·h+?D©JÃïX#?Z·x'/«y?D©JÃïX4FGL J1012.7+2439?í ¿kÑÞ@K0ñ€
|[À8¥î'):ŒÀ;ç(Ag©]@µÐÍbsé@ZA*2?¤.OÊkI?Á¼£´Ð'@æ<à[@aÓNq'?¡-àõ	¿àlh'î¿ãàoa6Ñ£¿æt -œñ=¿ì‡!œ1ú¿ïÿûÞ]BüAGNfsrq3FGL J1012.6+2439MG2 J101241+2439?ïÚ:'cÓ­?uG+O?râ·N*K?uG+Nÿ?ïäÍ\$É ?Šp¾ª
¸R?k2£Û6àª?Šp¾ª
¸R?î†*ÖӚ?œQ·\WS?§RžbÆY?œQ·\WT?ïò;D
pþ?KÝZåÁP±?[‰wåè?KÝZåÁPÁ4FGL J1013.3-2551?ïð¸Ú>¶‡@8Â÷ÓÀ:¬l){À<L-ë˕•@Œ	K¬Ò@'óUÎ?̚Ïú~¶¿?á=ö¬m²@ø"5´í³@eyœÞ?~[lƒr¿à×ϔþ)f¿èxQJuo¿î|?k¥À¿ïÿÿ" 5•?ïìÝxìzèAGNbcuPKS B1010-255?ì+î+QÛo?ÂïX=w?¾ Ž¥q$"?ÂïX=w?݃WôҜZ?ՒŠ@F™?á>T–±Ò?ՒŠ@F™?á~Kë'"?·Xhðò?Ýh)°Ùð?·Xhðò?âyõ&U?Á†æ‹K"?Û³UéÙ?Á†æ‹K"4FGL J1013.4-4006¿í¦,´üªt@*ÆÜ~ñw§À:z6ó²äÀ<VL¹6£@]U¼ú@â@ÐO8?Õ7¹«?Á§ßÐ?ýxZŸˆÆã@Aï"¿ïðõkQ‡²?ïmÅÖ8†Y¿å[¿¤Q¿Ûìü=3g¿ä\°ºv¿ïÿø¨ó©°AGNbll3FGL J1013.4-4008NVSS J101319-400549?ïë
Š…
ø?haöq'Ù–?dòuzò™?haöq'Ù™?ïæ¼Éç $?….'b#G?iC6ßÛV?….'b#G?ﳉõ_4E?ƒ|+¢|¢¼?ƒ'¨2î¤?ƒ|+¢|¢¼?ï,b+Ò|a?‰"æÜò'?šsº…°sý?‰"æÜò"4FGL J1013.7+3444¿Ì-oE+ö&@KÉë têŽÀ:2Ÿ|àÀ<o©æ÷n@,­c%`@!þÍ?¹?½CW¾ä?ÀoU®2X@YO?Ù@R5£zîß¿Ó3ўm¾Ê¿æwÏz&6Ë¿åÙ¾bPØ
¿êÀÄyA4¿ï÷?œÎ€?Âø<èÎdAGNfsrq3FGL J1013.5+3440OL 318?ïõªåa®?^U²ùâ?T«ú5<¦\?^U²ùÑ?ïü*ßӖ>?Q>q¯êŽ˜?>©cNÜ?Q>q¯êŽ'?ïÖàV¸Õæ?rÕ(ݘ`Í?tÔ£•\?rÕ(ݘ`Ï?ïáVÔ@À?\rŸ4''?né©+¿?Â?\rŸ4'}4FGL J1014.3+4112¿ïÕ¼Ì2M[@K{š¿4À:'7褙¨À<"þ)f+@{"Œ¿k@	ÒaaCè?¸ºt_Mm¿²æ I»O?ön"¸‰Hé@$Ž³°F¿æZùý‡€¿ãŒ¢~š¿æÈZý|˜¿á7ÏÆl`¿ä"'É›À¿ïú®‡ggîAGNbcu3FGL J1014.2+4115GB6 J1014+4112?ïþ[ÒRh?'¸,ÕÒb?*BÞÚÙq–?'¸,ÕÒh?ïûț6‡?Wàalos^?@ݓÃ%ê¶?WàalosZ?ïì|G"ó[?fjÂlQC?cƒ¸l¤Ù?fjÂlQ>?ïêáäöéÀ?Uýs›DbO?e	?ˆ?Uýs›DbF4FGL J1014.7+3210?ïñd³¹é(@Kâ­>'À;[HŽå
±À<ÓESÇ'q@ x|l75Ì?ö»Ò©…Ÿè?ÙV»"«P¦?ØmAKúªV@cS;ç6Û@¤tz{FG¿è…¶Æ'¿éÛÐ`U*T¿Ü€("X"¿¿¯'ÿ'¿âVbýüÁ¿ç½®(`qAGNbcuNVSS J101445+320725?ïþòƒ±??$$߃a? ×ÏÄì=?$$߃a?ïü-çËè?TçÞWè²?>Á§Ë»?TçÞWè²(?ïҏN4àÙ?|M0¢Â?v¸X叓<?|M0¢Â	?ïò«Bâš?M-±Ñ	?Z©z;üÐÏ?M-±Ñ4FGL J1014.8+2257¿îAË·ÿû7@K7=áâއÀ9þ†åÀ<XnoId@=!¤W
@Ũ¹?º,Ö¢¹}æ?³yHÁ9ñ"?ò…×Û(@ûRK§HY¿ÊœdzÓÜ¿åfâÂØWE¿é¬u>p~¿ïφ»p"?àË1¡ã•¿ðAGNfsrq2FGL J1014.1+2306OL 220?ïú¿û‰8?P¶ˆ¿k¨Û?EÍÛ"n?P¶ˆ¿k¨Ù?ïújQô›æ?XÝØ£–ö`?FV¸-ld?XÝØ£–öd?î¬á«†n?–‹"ô·e?¥1åGŸ©?–‹"ô·g?ïÚ^—šµ5?ré{ɤ´í?rд2¥f=?ré{ɤ´ð4FGL J1014.8-0537¿î'ìx1£ó@Cúãq*À;û
͹\À<'@eJÝt@¸'r0@=ø{§@K?˹€ôM?¹Ç‡þç|&?íî/ªèv@hÚPCs?íÑóbb˧¿Ù3œÆtÄ¿è@ ìߑ˿Üñ±Þ‰ã™¿ë;<¡Æä«¿ðAGNbcuAT20G J101446-054049?ïû,×Ljþ?@ÈÍ'êv¿?CL¢ÎTÓ?@ÈÍ'êvÌ?ïûn¦{ír?^	Ý-œ]?BEfJ<ô?^	Ý-œ[?ï¹åHp¡?Ð>ÜzB?†­ãÿ×w?Ð>ÜzD?ïÁN:MàÉ?hð³"ƉÚ?XâÙœ?hð³"ƉÚ4FGL J1014.9-4508?îƒÓΪ2@"Ùº=À:VR,†À<5'Í»à@	#Îç.M@bE¿ý±q?¹‰M-ZV?¬½™P?ò_äÓSÐ@)Ó)]F'?×ÅUŸ™¸Î?ëàÜ^e;¿äV$ßÞL|¿è°d‰Ø[¿Ö}ÓLKˆ¿ä¼†~3â†AGNbcu3FGL J1015.2-4512PMN J1014-4508?îçdĀÔ{?¡;ØqÇæÙ?¡‰³·ò¸V?¡;ØqÇæÙ?ï´«·Ã?¢z–ÈZŸ?'Õ;¼ÒÞ?¢z–ÈZŸ?îº`Uo©?™_–`'W?¤^éú©j?™_–`'W?ï8céb–?†f°Ñò!?˜óŒBÓ­0?†f°Ñò 4FGL J1015.0+4926¿âN
qˆ@J[9&A³À7!ÄÐoÀ:ùxiž)K@¸>Öªq-?ûþ/Egé?ŠžÔí?¥ç¨ß÷eÁ@WØåó@Yy&1—þ¿¶!x˘Å3¿ÔñëÀ-@¿ÛOqtõ¿Ú"fÝ.ĺ¿àޕÜär¿ØñnØ$ï¤AGNbll3FGL J1015.0+49251H 1013+498?ïþ±«{¸? { G\…?$åOèD•±? { G\Ó?ïóg 2ª?toÐ2f'¹?Yó0¿š«?toÐ2f'¼?ïÒfÌeþJ?€šÿj]Eä?v̙ÍÛ?€šÿj]Eä?ïø‹µÚ?>T.Š[ùt?Mӟ'(''?>T.Š[ù™4FGL J1015.6+5553?㓪ú–Lî@HûìÃã?À:`"ՔÀ<®¬&dØ@vÀ7=.	@Óû¶Å$?¼3Øt »Í?¾šNʓb?þÞüz9'@ñµh'?ïõd›‹a¿ÕUšü›¥¿è2ø6#¿åEŸ¶´2¿ïÿv½Ì~É¿Î$¡Š~ɊAGNfsrq3FGL J1016.1+5555TXS 1012+560?ïöâ¢Ub?UãÂ\(Ç?R:»UÇ;<?UãÂ\(»?ïû§†CF?TƒæøIÙÉ?Aaæòç¨Ç?TƒæøIÙÁ?ïzˆ±VÔq?ŠYuñšG³?®éÕ%qÞ?ŠYuñšG¸?ïåñá'B?Y宛yW?jä}½-?Y宛yT4FGL J1016.0+0512¿ã¸™5]2@Gƒ*ZFsÀ9Ó¬ºÞŽÀ;ô{/PP@/Ô®Bž
@¿û}º@?§Å#yñw?Œ¥'ÛÃ?ãŠ
jKÎ5@ÇÑb³©e?ï k°RBÿãxQ [ª¡¿æpÒÐòÌ;¿ày7Ó¬¿âAØ}7¿ê'õ¦	êeAGNfsrq3FGL J1016.0+0513TXS 1013+054?ïüÙÿóù?2ýâYŽl?97 `6E?2ýâYŽ˜?ïüâñh?SJ÷kQ[?8èwl¿7
?SJ÷kQP?ïíL}û‡3?mz,Ÿ0?b³'xÌE?mz,Ÿ*?ïÿ󥩦>Ñü¢<MN=>Ø´¬³ÑOv>Ñü¢<MSc4FGL J1016.4+7703?ނºg'6@BmÏÝ"…fÀ<€Ä"(ï
À=§s³VB@!À˜ÐÆ×j?øêܝ$h•?áŸ!"OX?ï2€áü}@	å¨ÃÙD@ÐEìO¿ïÿ.ÿqå¡¿×2ê£whí?ïÔ*pìÒ¿¯ÓÏAé{Ñ¿ÙÕõ?‡ªY¿ïÿùŸé"ÚAGNbcu1RXS J101647.6+770239?ïßÿ"õx?yøL¤s9?p}6C=?yøL¤s8?ïÇSº¼?"Ë4¹ß6?|Vt"¡ù‹?"Ë4¹ß7?í薀ÔýÑ?¡®ÕƒwÚ«?°»KùXy?¡®ÕƒwÚ¬?ìf
MšÒ?°鳊%
?¿"Ï•")s?°鳊%	4FGL J1016.5-2650?ÕY†X Š@8oawêiÀ;2üÁ‡À<¥D@¡°¿@ ýçP[¸
?ÿ'6¾ØîC?Ôï˜ß_vˆ?ζ`dCÌ^?õr-å˜î?ý:¥¸‹Í(?î'ØÚø¿ïøžwNëö?ïÿ¡Ö~ý6¿Å¾´Ü?,¿ìè=Öû#ø?»¯d9ÕåAGNbcu3FGL J1016.9-2653NVSS J101634-265057?ï×X&¯;D?pòÛ ®Í?tSì¨b^;?pòÛ ®Í?ïÎBpjT?'F¾.sU?xÞÇ·ÊÕð?'F¾.sT?î{goÞÿ?š!w­"¦?¨I‰p#?š!w­"§?î\TòAh|?Ÿv›¢ú¨?ª:°Ûéx%?Ÿv›¢ú©4FGL J1017.3+5204¿ÛÏj怰è@Iü¦\ö{À;†ì"øø¥À=š‹1!
@ ¦ß¢ú@?úpŽX÷ˆ?ÓCâb¶-¤?ÔÄO»)6Z?ûj÷	·8ç?ù&¹Ã_¿ßW7õ9Ó?á£&`;ÿà¿°Xߕ&mR¿Öƒb¯É¿à¨Ž"'Ùd¿éҜŸÞW9AGNbcu7C 1013+5217?ïΆ̷…5?uÎñ‰èZ?x¼™¤=f?uÎñ‰èX?ïâÿÂå±?~¬¶rãc´?m=NöG?~¬¶rãc³?ïqÅqG.?ŠŸÆÌ 'Z?'ÇQ×=Š?ŠŸÆÌ '`?íwŸEÎ?–Â-稢'?·C]ѓ?–Â-稢'4FGL J1017.4+2538?äÙ÷57?@KÏ\WìÀ;Î²€À<ʴĘJå@#mükJü©?ñxá'ͤc?Ù~íEé]?Úu$²?@Áù£Åm@¬3ÁM'°?ï»U
ôOÉ¿ïæòåˆ[¿ïÿè«î0?ïÿülò¿ßÙ%ÀÙÏj?Þ"ø!å-AGNbcuNVSS J101724+253955?ï÷žD2?QCt.[?PÂýçwœð?QCt.[?ïé#Ã3ÒÕ?'wž	2+—?fÜ<Ì-*´?'wž	2+–?ï ³Žåò?‡ L›"H?‡àFƒ@?‡ L›"H?ïæ蘕Ø?i´shŠ*Ö?igjù'?i´shŠ*Ô4FGL J1017.8+0715¿ÔïmŒ,@HGÐ|"µÝÀ:´ÿK¥À<N°ªWVÿ@·ê)))@ÎɟâÚ?ÉIO>ׁ1?¹þ_ýý­|?ì>m=ðüW@
QÃu‹~?ïûŒž"#¿ç?*¸:o¿èÒ¤Uµ>¿èiʞõ#¿ïô£
[£•¿ãú'®š²žAGNbcuGB6 J1018+0715?ïþÚ6o8³?@ӐC£?"\™tåª?@ӐC´?ïû	Ý?`0´*3=?CØE-è<?`0´*3??ïۗ9¼âË?t)ƒB¾À?r4c!ŽšJ?t)ƒB¾Á?ï×g™h‡T?aÃø"©é?tL3K¼V.?aÃø"©æ4FGL J1018.1+1905¿ç"G¸S;Ö@KÉÙÓEÀ:xàU¬ÛÀ<"eByø@FOo©Ü@˜0LÎæ?¹F½S³{¿ d¬Á®Ox?æîÆؤ@	rmœ™ì¿Ù·
bZé¿åçZíŒ_õ¿áá›@bƟ¿åP—&ø'M¿Ëªø;»lþ¿áTHÏAGNbll3FGL J1018.1+1904NVSS J101808+190614?ïýkÕe?3"¡Š¬]?7§ÑTÖ¼?3"¡Š¬]
?ïýn'¡•'?Oa8FÑÍ?4‹róSñ?Oa8FÑÌ?ïòæÌåFE?i¥É8@ò|?Z2f5svÈ?i¥É8@òŠ?ïü8_¡‹Ž?0–2*ÿK?>=ó£•E?0–2*ÿY4FGL J1018.3-3124¿ÅM_…W@5ÕW2À9´¸ÙÐÁÀ;òŒVºø@zõ }ùÖ@°1;nÉ?ª
¹|
¿?®ƒ
¶è4@	Wɱ@iDû‡ H¿ºNnxƿᦕ€…K"¿è¸Ëž#—	¿ç×"'$€¿ì3bƒþ¿ïÿò(¦è7AGNfsrq3FGL J1018.4-3119PKS 1016-311?ïô[`¸ª¢?T"/H¯}?WI>Žª¼{?T"/H¯p?ïð^¸Å':?yéZ@–!á?_BŽu±ŠË?yéZ@–!Þ?ï¤iT°í:?…g8ò{:,?†åªÓı?…g8ò{:*?ïíÅtö•?P윸R[æ?b€:‹	jº?P윸R[â4FGL J1018.4+3540?ïýe-e1@L=
à"S.À9ÌQþ'BÀ<i­1üÒN@ðÇP6#S@G³zì/i?µÕRWeÂ}?»8­ªÑ$?ÿ»ê&z@±~Rû¿ËžM]€ä—¿áݑ`eŒ¿è« —ºœI¿æ@>-b9¿ïWàyQû¿ï•ÂH"AGNfsrq3FGL J1018.3+3542B2 1015+35B?ïýÔ¯j´å?;"ªáxÉ?1Z"ªXÕA?;"ªáxÆ?ïûÞú…=?WóµË7ˆ?@"¥ëa?WóµË7ˆ-?ïËQèJ´R?|5ìߍú?zWÚ¥Ö«?|5ìߍù?ïûÂÝF±??2†£Üv29?@ôŠå;î?2†£Üv284FGL J1018.4+0528¿ÜÈÙo·ª¼@GÕËeè'À:,ßØBKÕÀ<öó4@O-\¯ƒ@uð¥)?ÂN…7x'?¸¨*ÕÁ"?öš۸ù@†ü®'ÎI¿î¡¢7_é?ïö€Z-s¿ä
Ÿ¥Í/¿åÓsD›:"¿áŒ	XnV¿ï¬¿EûŒÔAGNfsrq3FGL J1018.5+0530TXS 1015+057?ïòá1€?a‹–úq8?[æ=œÿÜÜ?a‹–úq8?ïû·$eÜ?Y§P|ú?A#çnhŒ°?Y§P|þ?ïqJ4•?&TÍ·ô?'Ö¹~­$?&TÍ·ó?ïÙ¿z¹rÖ?eeÎ¥FEË?s B£F"Ü?eeÎ¥FEÈ4FGL J1018.8+5913?éM9×ñD@HIÚßµÝÀ:›&Š®DÀ<Ì_‹€Ò"@¥¿â®‹?ÿ•a%´Å?ÀòBÒãg?¾o/êÖ?ÿk/=Û,â@{Ùs¤<‹¿Êk¯¦vKâ?ì	ÒÄ]"¿âvIh(ÞF¿à©RtA}¿ßˆn ¿ïÿþBe«+AGNbll3FGL J1018.8+5913TXS 1015+594?ïëü"‹®?fˆL©÷?dktQõŠ?fˆL©ó?ïíÆ&ž¿½?xx'*?b9Ùa@A«?xx'*?ï«ÚóJl?"ÿH'ëÀ?…	O-dº?"ÿH'ëÂ?î°xþ¾¾`?¤À­˜%c?¤øp?¤À­˜%d4FGL J1018.9+1043¿è?VxíY7@IMæ`ɊÀ:ÆIéXÎÀ<f,§þ·+@Éáš9R@·S´Eí?ÑĬ{*C?½è""¨¿?én
ŸOæó@—©Tw¦¿äÔ§Awï{¿èôúþ¹Xý¿èú³$…‡¿ìÛÄanYû¿ð?ïÿ—ŸïI$AGNbcuSDSS J101857.97+103625.6?ïþº¶l?1ÉYXÚk?$^ôž¹0 ?1ÉYXڋ?ïØ
ò•FÞ?"Ò'‡S"?sùµ\'Z?"Ò'‡S$?ﱟ²¯j±?Êx‡Ó¤?ƒ˜T%Sú?Êx‡Ó¤‡?ïÜ\ë·bì?jÙWSG
{?qъ$N‰~?jÙWSG
}4FGL J1019.7+6321¿Õ®çéYàG@G % …²À:h!È`À<'ž1Ún@‡-nÎõ?ÿ
ýÌ=[?¼]Ú{·?ÉgÒa·*#@؎6F@"‹½¸Þ?îísk1§B¿Í¶†9j"Ù¿ÞMdºã¿áŸ°9F¿æ˜f^ꖿðAGNbll3FGL J1020.0+6323GB6 J1019+6319?ïâºg{#?ka]Wxkø?mE˜"üۗ?ka]Wxký?ï÷óCør5?aÔFR´S?Px"3?aÔFR´Q?íD•à¨×?©'Ln½Ë?µÛPÿB¹E?©'Ln½Ë?ïŠ|ª–·
?qªÕM½ð•?`ÕZR<–?qªÕM½ð–4FGL J1019.7+0511?Ã0П՞	@Gâك"t—À:áüjIJÀ<pšäó4@@ Œ£jRÚ?þú¢
¢?ËÌÆÐ&?¶IÏAq9~?íM	""}Ì@
!N§-¿Ø©Ý´{/¿æÀaïß Œ?¡x­™W¿ÖÞ¾fØ|-¿Ú<XüŸ£¿ê<þޗÐlAGNbcuNVSS J101948+051327?ïÿŸÁhå?VT[zŒ?˜¥Æ±T?VT[{Ð?ïýD³qM?OÕƦÀ%?5ߺdu"ý?OÕƦÀ-?ïø»g)V_?a8¯ ¼?McZ¦?a8¯ À?ïûôwﴞ?,Ž<w}˜²?@. A-‡o?,Ž<w}˜¡4FGL J1020.7-3920¿î&V—¶{5@-¥ê«%)À:õgXÔ­lÀ<"UàÝ%
@ dæÃC?þ*™Eå½?Ê÷ JÂÌ?½Ù!™Ø®­?ôä$7í'@ÜÛNšÂ¹¿ïÜ>Å7­?ïâÉ¾²¿àِ"Š¼¿ÍOÿ‡4<H¿æEz=]Ùz¿ä¥ ¸ò¥AGNbcu2MASS J10203893-3920563?ïý˜¬"T°?0x\÷ò?3:›ÝZƒG?0x\÷Ë?ïì[V®Y?‹
Ã×ès!?c÷¤©Q§?‹
Ã×ès!?ïëœ+­Ú?fvZ•¾c?dcÔR%q?fvZ•¾c'?ïwœ5ËÃ?ïÜdíð??'yN‡Ä?ïÜdíð;4FGL J1021.1+1626¿ã€Ñ9˜œé@JÕQa£ÊÀ;cüÈ=À<ÇG&/>²@ Ô±šA_F?ýàA8¯sö?Ó? ^¯¸À?¥Ïƒºþ?Ëáºö¶€@nÊ£|ÇQ¿ïÿÇ*Ì\e?ïÿ<‹¡‰R¿æ‡9zu$¿Ã¢ÓÔþÊv¿å­å˜îy¿Õ¯=oÍAGNbllSDSS J102100.35+162554.0?ïþǯj×?S¹­Žûy?#…	R™¼?S¹­Žûa?ïü),ƒå?]7XÜ¢¶Ñ?>¶ŸÓàÚò?]7XÜ¢¶Ú?ïð±e—"+?]Ä_ÈÏ ?^4ÐÙ«
?]Ä_Èϔ?ïÜu|{†â?biÒtá~?qÅAÂ<ŽÉ?biÒtá"4FGL J1021.4+8021¿Ôi»ý¡‰@AM˜ˆøbÀ:W‡¦RÀ<˜ƒÛÂ3@"¸_˜@vWu1ÛD?»î›~¡Â?ÅӊV/·@~ɄBð@?üo5JÁå¿Ú¶ÇÝyÃ:¿ßWsÄÈÇZ¿ãd.]‹vk¿ãºPþöſ×øz?Ϟîm0…AGNbcu3FGL J1021.8+8023NVSS J102201+802350?åÉÊ2I*%?ĵŸãšÂ}?Ôlk›m«´?ĵŸãšÂ}?꛴ɍÓ?Ï+yvä¶?Çõ',ÙÈ·?Ï+yvä¶?ê×4·ôgÿ?°rÚê`M?Ä£- .`?°rÚê`N?çÌ'j¦1?³Áx…°¦?ÐgàÛ*³ž?³Áx…°¦4FGL J1021.9+5123?¨O\›˜@Jt×I''?À;҃9LÀ=Š'¥aN@ƒ{³žÇ?õ¢Œ¢:R?擥cÒ7p?ä³øà¦ôK@¸d"@úø´‡0¶?徚À
F«¿âs1fªY¿ÞçÂòXx¿Î û;;¿êFJ'Û¿ïâ~
ÇÚAGNbllMS 1019.0+5139?îÖZ?}óC?Ÿ!J$§
?¢š\ Ëð?Ÿ!J$§
?ïëO2[ˆ??"+ï"äj?d°Í¤wÀÚ?"+ï"äi?íè3°fÈ?Ÿtk»¸©?°¾b|É¿"?Ÿtk»¸§?îül—*_Ý?'JUôªÖÚ? 96Z#?'JUôªÖÛ4FGL J1022.4-4231?è 06Çqß@(¶Žæ¸0^À:\a5¤ý{À<^~ø-£§@4Ö ˆŒ@ª"£hO?ÀºIýÏùþ?µÏ?Š?öFB‰èK®?þ¤ŸÔò
I¿ÜÅÄDèè6¿Øä2"Œ—(¿äU.enâ¿á=u×H¿â°T[¡çF¿çYº¼)›AGNbll3FGL J1022.3-4234PMN J1022-4232?ïÞvv!4'?hÄ_ÚÑ#?pÄÄïe¶û?hÄ_ÚÑ#?ï"6!©É?á#æí°K?Šòw•ºG?á#æí°K?ïÄ^,ô?UÅWI¬>?}ÿtP醀?UÅWI¬??îÙÕêö?†øyEV™?¢cÆ¡^€š?†øyEV™4FGL J1022.7-0112?ïhžHÑ9õ@F08⟜éÀ9˜püÀ<Sq@€bÐãå?þY·+zØ?²ã2½—{?¥(+Ã'\?ó{–^{¶Z@ôœ"µâ{¿äÓF=üåÄ¿á¹\þØ<¿Þ2½—z°¿Úv7_ÞO¿à‹aÝ냿ßä€]2‹AGNbll3FGL J1022.8-0113RX J1022.7-0112?ïûµMB?;úO˜|"@?A*Ê÷ó´?;úO˜|"R?ïûâ"?Xڊ±"W?Cûÿøu²¦?Xڊ±"\?ïç
Íæ?qeÏ·G?hàò2ôI?qeÏ·??ïª§ÄP?rWmi²Ý?…|ùÖëV?rWmi²Ý4FGL J1023.1+3949?Æÿ&ˆs'Ý@Lo1½èÀ8ßÉ#ÊàdÀ<"àæ_E
@ŒÊ(W¸@ùÅS[È?¤L/¿œsÐ?»'Æ€FP5@ä­Ýô<}@ü9§¿Ì†ùXñÞª¿áíÁ9ÓÁ¿ä'ÙaÏ©¿éDåw¾}¿æV†''>¿ïÿúŒ—ÓAGNfsrq3FGL J1023.1+39524C +40.25?ïÿ‰"§r?*¨¯`%?͋®E?*¨¯`A?ï÷"µ=$"?kGÛ<"ö?Pö•…¶Ûó?kGÛ<"ù?擄äfòâ?Š×XÜ6ß?†ÓÆæCG^?Š×XÜ6ß?ïÿç!ãû:>à·/¶Åˆ>èÞÆVŒ>à·/¶Éµ4FGL J1023.2+2859?ï9U®ò×ü@L²82vtÑÀ:ªÐ»nÖwÀ<Œdý±@xšô¬·@uX'?ÏÕ£5#Î;?Ï?/*ee?þˆýՃU@™½Uá]þ¿Ú0œ_ǐοÝ&‹º³Å•¿åâ,m®"¿í½mHضæ¿ÚØïþ¯¿ðAGNfsrqTXS 1020+292?ïñÉTYa·?g¼FØÍí?\mWM<"?g¼FØÍò?ïöYŸ@?o†À8Û?SLÁÁ×Ô?o†À8ä?îLHKæŽ?œVº3"Ó?«;{A—?œVº3"Í?ï¥9Ûb§Û?v-ÑL?Ù?†±‰'V	>?v-ÑL?Ù4FGL J1023.8+3002¿â\9}N@LÍ®>lLYÀ;)€z䢬À<µb+nBÔ@!7¡¬ãx?ý´òd/U?Ç}ÖZHŒ?n­àMˆ?·¸Ñî×@€Qû,Ý?ëÔD$òþ¿ç³VÚh¶¿æg¾U:Å¿ÒÙ~ —O<¿Ô¢ÃäÆ¿¿à§".ÍüAGNbll3FGL J1023.7+3000RX J1023.6+3001?ïÿ@ÛþZ?
IVW‰ ?þ$€4¶C?
IVW‹?ïý"±©?K³ ~°…R?3ߚr·i?K³ ~°…P?ïüz'kH?8sž "ó>?</+l¥ÁM?8sž "ób?ïûxÐðU?1ód3cÅ?B¼?ò©¹?1ód3cã4FGL J1023.8-4335?ï¾nš`wM@'3ó.ZÀ9"Üõ)À;¸•Ew–@ 
½Ál‡?ù¬gíO#T?°9?硏\?¼ßyLȼ@ º}>ð@¥['¡'­?ï÷=Bÿ¿‹â꬗ß@¿Í/?ɸ3¿×•)<ºEŒ¿×úžAI!¿ÜÞ&¼W^·AGNbll3FGL J1023.9-4335RX J1023.9-4336?ïüÝ"á+?>iE‹FÅ?9Xö§6?>iE‹FÌ?ïÂeqDÈ?š´¸˜'}?~ÍtÇ]œ'?š´¸˜'}?ï³Ñ]vÌ?†ÝP™¡´Ø?ƒ¨ "LÈ?†ÝP™¡´×?ïTž‰µ
4?³ž*§¨|?•l.É^¹~?³ž*§¨{4FGL J1023.9-3236?ï÷ø5™Ã@4½Þß)À9høH{™ÔÀ<h;R¼@ÕÈ<DSí@Yú—á2µ?°¡ŸL‹ôÀ?¼ODyׇ@ "Ú@¬Ûù Ý¿Óå•ñnlÅ¿âã}_*Þ¿ç‹1÷ÉЙ¿å¨âaßn¿è¤Pwؕ¿ïÿ܎᯳AGNfsrq3FGL J1024.1-3232PKS 1021-323?ïýØÅI­A?0¯ø}Â
†?19Õ²•øé?0¯ø}Â
 ?ïúó
0,?W¶¨â"Et?D3ÿË?O³?W¶¨â"Em?ï©Ü"(?á¦ý?…ˆ÷[õÜ?á¦ý?ïÿ¡œ$N>û8E{h‹?˜ÿvìng>û8E{j"4FGL J1024.8+2332¿î8Œ§ý2ê@Lf/¾3¬ÖÀ:Jº))À<'ÜÜåHÅ@ex?V×þ@Ë\ŠD'?¹ÁHà®ø?z™™øÛ?¿¹:^J¹@0g…JW<¿žóÂbe¦¿çy€‰þ#¿â˜ ˆ5Ä¿çJ†¡oPñ¿è_ÊÀØøª¿ç_·¼]êAGNbll3FGL J1025.1+2333MG2 J102456+2332?ïçNi'"ë?f¹F‹¹'?h±–}{?f¹F‹¹+?ïû£#ç¢?]ü a3Ð?Asûpar?]ü a3Ù?ï̌º‹W^?|57˜iÆJ?y¹¢ºTR?|57˜iÆI?ïâ|1'4v?\ÎäÞO'?mƒÎØˊ'?\ÎäÞOþ4FGL J1026.9+0608?à±ivDC@HãBEõ­—À;éuyÿ À<…/PO¤@"êvÖËÿ?úG«<#?Ƨ0›~K5?™:"£§?Ó/á»vc?ýÄL`*ã¿éøÍ ¯¢ð¿ï—eýŠÚº?èËb¿gßb¿åÉ8Þmß?
^b`ó5¿Ï¸fGÐAGNbll3FGL J1027.0+0609NVSS J102703+060934?ïþ6ô¨_F?2ùÃKñ?,µz"œ?2ùÃKž?ïý‰÷?L5¢çßa?3·CÃ?L5¢çßa)?ï崖ªa‰?lä}¬é?jKiUžv}?lä}¬á?ïì"프¾?Yf–¯äID?c{k{A)?Yf–¯äIM4FGL J1026.9-1749¿ï†ŒP'@@',ºs-õÀ8ýN.KmÀ;ށOøÄ@¦'¥¸‹?þ™‹Ýtk?¨ý?l®?Ÿ-ڃě%?ôÈØ앿ð@œÜ$¾¡?ïÿ"­~ÿ¿âöq ~¥¢¿Üœïd|Vh¿ÜÂܾ²W׿ߣÂèG|–¿á[íœP-?AGNbll3FGL J1026.9-17501RXS J102658.5-174905?ïÿ‰Äéxþ?•RJ°°Z?
ŽÅ¡À3+?•RJ°¯@?ïýŠÍøI³?H³(…Ç#?3©=²^s?H³(…Ç8?ïê/àE?mõ¢°%º?eÐo»?mõ¢°%º?ïþ}Ž?®õ8íKÎ?&ø/÷#Å?®õ8íL94FGL J1027.0-8542?Ãóû'lñÀ7£é·¿ŽÀ9VFíû¾À;äé@- .Q?û£®@˃?±«bï¹`ß?´×mÌ ª@PÕ¥¹b?ë@­3J¿ÕTF=Ñò¦¿à@GD¿ÛQ'Ã'ë¿ÔÁä×Ût¿à(»àì?¿ÜœŠâAGNbll3FGL J1026.4-8542PKS 1029-85?ïàƨ{Àc?p
Ú±ŠÆ?o9W"?œ6?p
Ú±ŠÈ?ä¥TœØ2@?ÔThŠ¨9?ÖµVÆO›'?ÔThŠ¨9?îu"àèw?š•îÐƉ­?¨®&Áñx‡?š•îÐƉ­?ݵn™3?´ìžKc
?á%Hñ³f~?´ìžKc
4FGL J1027.2+7427¿íUÖ.8@Cšù jn3À9Pý^e%À<gŒSã@rªuÛy@;'}E¥ü?°F[®ýY?µFÏóî@g‰¿1×@.[~?ëÖz•ÈSÁ¿ÚOŒ…4î¿æ!pÞ9†´¿äñ"íjÒ¿è…?\ŒH¿ëKã-abAGNbcu3FGL J1026.5+7423GB6 J1027+7428?ïò·ÆÊL?S	" Žú?Zsîkf"?S	" Žü?ïúgÑæ7°?h6øÆiµ?F`¸g!>>?h6øÆi¯?ï]\öŒ† ?Š.ªZXÃ?"Ta.o;ë?Š.ªZXÇ?ïú_»>?:ß"‰ÀF?Gâ"?:ß"‰Àq4FGL J1027.6+6317?؂C«'‹@G}"M:"À:;ðJ€VÒÀ<¢w$ú‹L@²' V!J?þS¢úkk‰?¸ø*We?ª®NÝ]¾¢?ðïga8)<@lïåU¯µ?ïû=ù_ÒÎ?–'¿§í'¶¿ä¹xýAߞ¿Ñ>sV¿áƀ,‹#¿ëùsôÄb›AGNbll3FGL J1027.7+6316RX J1027.4+6317?ïóÎt´À?TÛˆêÙý?Xcܖh?TÛˆêÙì?ïó¿Õtöq?mÓIeae?X€UÜ?mÓIeag?ïÈ/$Ä#€?}á¿QK0¢?{èmî?–?}á¿QK0œ?îàhZ<˜q?‡"ýÕÅ:{?¡ùz\6xõ?‡"ýÕÅ:z4FGL J1027.6+1828?ïÿ6²9X@Kñ«ó8qaÀ:zXËs0yÀ<u¡Å¸•@œ_.
Ú@ÕIe¤Ÿ‡?¹ÎAÒ¿ªê^ƒ"â?ð­
ê¤@є\Ãп×wCÃÏ"=¿é"iÐË¿èӓZ»7y¿Û¢ëý¿ˆì¿ããðj`Æê¿ðAGNbcu3FGL J1028.0+1829GB6 J1027+1831?ï÷.8º7?T¢ ×R?Qû£Ž‹"?T¢ ×T?ïæqc
»?ˆtöã%¤;?iŽœòDìR?ˆtöã%¤:?ï°YSò¿©?¾"ÝÚ–?ƒé«Pµ?¾"ÝÚ™?練ó;âz?t"ZĂ2?…š1a‡?t"ZĂ14FGL J1027.6+8251¿äß䆥x@@hó¡LìBÀ:Ž‡=vƒÀ<¾|ŽÆØ@^Ç»ëÓù@é']e5å?¼±]Z¤k¿ò»Úó<^?Ôå¢;~±6@-W&,¿ã{ŒhX®î¿àèh~ïtB¿äiæ÷mŠ¿æ<Ý5Мe¿áe¥«ö"p¿âÖ ž9%AGNbcu3FGL J1027.8+82532MASS J10284195+8253398?ïüÎ÷'W}?7‰²yÍÛ	?9ˆCmDA?7‰²yÍÛ?ïþtô§]Ñ?BÃsŽa)?(°µŠ"è(?BÃsŽa?ïë$°Ÿcß?lßËup´?dÛO`œ! ?lßËup³Ü?ïý€°šBÑ?#_kâcQ?3ú{-ép¿?#_kâcF4FGL J1027.9+0252¿ïýùÓj@HÏÃøÀ:nӕ=êFÀ<A†l–+P@³¡ÀY¡Ý@õ±…H©½?¿ÿ²RM)Ô¿µ
…†H?ò¡öKKX?øâ£8SÙq¿ãa|¢¿ëZ¶ÐE®¿ìÐHbz¥¿¶d±Z€¿êê~äa"¿ïïK|ÖtAGNfsrqTXS 1025+031?ïß/Un¼Î?toíl·?phUH¡˜õ?toíl·?îyvi…÷?·Ëßæ¯Æ?¨o8™g ¡?·Ëßæ¯Æ?îöŽÃÈÙ?"]àQö? ŸÇÃru?"]àQö?î8ÊÃ{nÎ?£þ¨æ'd?¬sSÈI9?£þ¨æ'd4FGL J1028.3+3108¿áM7ÿæ@MOп "`À; ³	­'ìÀ<Â=U™@óF3@@÷U^×%ì?ÁÁŒ|Ћ¿—».>׬$?ÖÄzÃÀ‰@	¢ohî€ý?ècÆ
•ê¸¿¯Ù1½šÞF¿ç,$K8ãv¿á*`üš¿çN£Îç?È8ôhG<*AGNbllTXS 1025+313?ïùnG—{È?EvW2ösº?JFá¢àå?EvW2ös¶?ïýVø+ÏR?Q¢\^½RÔ?5H>¡…i^?Q¢\^½RÛ?ïæ8À\?oçûْ7?iÇ?â棝?oçûْ6ÿ?ïúM,"Z×?5HLÅäì"?FËM
?5HLÅäì¢4FGL J1028.4-0234¿ï‹†@FB[åÙäÀ:",Ý®œ`À<YZ;µ¸´@œ±a;.@}G{¿"ÿ?¼9ï:
?´«§Ž#ïž?õ	Ggž@
Õd]͐—?ãi§c†¸¿åvæF–"¿è2ŒÖ<¸¿çwlþ°õ¿ìð]ºpT¿ïñÈdˆ?ÕAGNfsrq3FGL J1028.5-0235PMN J1028-0237?ïû"'ê¥??	ŸÓ4ž?CuôVn??	ŸÓ4·?ïüõ|ŒaÉ?RÙaïipn?8Tœñ¶1?RÙaïipn?ïæT²b?j*[Ji¿?i«Màâ@?j*[Ji¹?ïê:›R‰?T ò¡Ö?eôÅd­w6?T ò¡Ñ4FGL J1030.2-8403¿æÛ¿õ¿˜À6:îA'šÈÀ:Ë£jÓ³qÀ<t±i@ k篧"@Â9櫛$?ŝ´†YöÁ?³Îð"{rg?ñBºtÛt/@Š²öâË¿ïÏAò×?ïýw$#Ë·¿ç	Ü!Ôf¿ãØҔŒê¿Þl¤Ùh¼'¿ä.1,edAGNbcu2FGL J1032.9-8401PMN J1030-8402?ïö÷Hq†@?L/öçQhc?Roó}Ï?L/öçQh[?ïêñŸ:R?"¾ÚÂ[ò¥?e`Åᮎ?"¾ÚÂ[ò¥?ï߀r£ÆÜ?pc;—nT?p?Æ®'?pc;—nT?ïB*éäßõ?…þUBÏö?—º¢Ãd{?…þUBÏô4FGL J1030.4-3001?î‡w…¬X @7¥/Ÿ¾wÀ:—F·G*À<Wé^ÓÊî@ú#d=;@ÿ\±Ö§?ljCu –
?À¸SÙpõ?õ'ÐɱZ@æ¼,k˜Õ?ïyێ0¯Ë¿è"^ß´[¿çÔ/—¿æÒ"!=¿ïÿ­_I;³?î47ûäAGNbcuPMN J1030-3004?ïÀ¡oåš!?§!Ý<c?¯H
2ðl?§!Ý<d?îþg3c90?´–ÙŽçY? ŒÉÌlü?´–ÙŽçY?ïr»ym3?‰¤É‹·?'¨ÒY¿?‰¤É‹·"?îìßávô'?'NƒÜF?¡2落'?'NƒÜF4FGL J1030.6-2028?ï(Èû'±@?s̪ï,À9䌎\À<.'"ø@ ]>6q?ûm±cºº|?ÀªQø›1Ê?º¸p^â¹s?þӊ¦·N@:㫶}¿å<O;§uû¿Ýg"s—§¿Ý–±Ý³$¿Ðkž3²4¿Õî¯á»v¿çø
¢gÉAGNbll3FGL J1030.4-2030NVSS J103040-203032?ïþïܚž?'¤øx:ß@?/'6V¢?'¤øx:ß?ïýAó?KvŒ<ÕÍ?5ðcÛe?KvŒ<ÕË?ïçì'–"?qÜÇG<µ?hØikê?qÜÇG<¬?ï㮯FñÍ?W—Úî@?lQP¹2‡?W—Úî=4FGL J1031.1+7442¿äz7LÎ@C™b¶®}À9×â[ªJÂÀ<7 Àiçû@ÒÛ¯"¬@j¶ÂŸLa?°/x""]¿ž¶eà¸À?ð_1£æúu@;ö%`¸¿Ú«Ä"o
¿ãóVµ{¿äÁ߇Oj¿ä¹mtw¡¿å°‡‡H^>¿'fU8Z~@AGNbll3FGL J1031.0+7440S5 1027+74?ïûAT)n¿?<çú³"J?Bú¯ZE
ê?<çú³"A?ïüá~A€?O°`¦È»þ?8ô•ô?O°`¦È¼?ïò9
¨"ÿ?eœ·àdõ?[ä®Ö$?eœ·àdï?ïòeD±"ö?J~ô«ö7q?[5vœØ€?J~ô«ö7ƒ4FGL J1031.3+5053¿ÕßåøvT~@K:\|ؙÀ9$wSôsÛÀ;ñEgée@ 'äõ8?úÑW%€Ã	?¨â¢:ìª?¦ÝäIk.@Ûh‹Ú"6@{Û3íÃ=¿ëdµ÷ž1¯?±¡ÙY"0,¿Ú¬)Ür\¿ÓÂNĉ1¿ßYvɋ¿¾|^pÐAGNbll3FGL J1031.2+50531ES 1028+511?ïô¼ÝËN?ZÔs·@|?V†Dibÿõ?ZÔs·@v?ïòe(èNÀ?x5¡=e9?[5®/bV?x5¡=e7?ï·ý¶³?ƒ'¸¶]¼à?''x8SO?ƒ'¸¶]¼Ü?ï!ë~å.Þ?…S°˜Ýç?›Â#Z$?…S°˜Ýæ4FGL J1031.6+6019¿à"øõ´&@HïÝëÙÀ9qÊ0:ZoÀ;ßþiýʜ@}'î°@ח{²(?³ dd?¡A¸~ƒ‹?ìEHßlâ@/]K4²¿Ç,ý6¡þ¿åh9Úí!¿æ9ÐÁN‰¿çk%@@¿èT@ßn:¿ðAGNfsrq3FGL J1031.6+6021TXS 1028+605?ïý
ʋe?+ëiÎ¥k?3‡'«¤Ö?+ëiÎ¥kœ?ïý£0¯Œm?F:¬¼j1;?2æzƒœ™i?F:¬¼j1?ïÉ!ÿC…?xæÄk0,I?{o^=pª?xæÄk0,:?ïýÖìKJ?#WŒÔâN?1HŸ}¥´=?#WŒÔâA4FGL J1031.8-2609¿è"€ˆò4Ú@;ÚÂXՄÀ;bÍÞDÄUÀ<©EW"&@!"«s5Ø?ÿUdìã2?ÉRß äçv¿'õžþ'U?Ëò{Gžû@=Ü.""?ïÿå(
eC¿é#´ùàV¿å"…fîW¿ÞTÊ\°¿Ùö¢½.ʿ͘uWEMAGNbcuNVSS J103137-260715?ïþüÌ)?Q·æ|Ò,? 3?þ}~:?Q·æ|ÑÍ?ïý×¹dAZ?QW'…c?1B4Ýõ+V?QW'…M?ïô{#ðj?aft!?W	¸,T?aft!?ïë¤&Öùk?S	'œh
?d[Ù)"Û?S	'œh
4FGL J1032.6+3737¿Þ/YÂ	ôÑ@M‹ÐÐgŒÀ9ÞHÈÆ­ÏÀ<O[ïêß@nf'†*@°ÔcšL?·٘b7¿}ËކÒz?DzvÊ·ž½@	Â*úÕsº¿ïðÝî]@M?ïû¾½?'¿ã.$5inY¿ß:;֚׿ã/×^ G¿ÚºTDzÙ:AGNbll3FGL J1032.7+3735B3 1029+378?ïý
›ÐDŠ?2ÍJ-åUC?7«!}Û´'?2ÍJ-åU>?ïüÇ¡B?Vl[|@Ä??IÂõë—q?Vl[|@Ä?ïî
‰Å?¶?g÷ԕ§%?aõv:ÀI;?g÷ԕ§?ïì_Üê?YR?P½ü?c p#øÕ?YR?P½ûù4FGL J1032.7+6624¿ìÏí–@F¦ˆabñgÀ:³Ò†ëAÀ<áN‡Lü@Ýòd@;bŸ1‰?Á-蛊_•?¶á@w>{?ó{X|˜Ø@&©b"?èø±Eˆ¿än"½"u˜¿Ü§A¼c¿â¿Sg†¿ä?_¼S-¿è?¸¢HiÑAGNbll3FGL J1032.5+66232MASS J10323905+6623234?ïûèhUÒs?7µ©´C'9?@^^¨¶6?7µ©´C'3?ïûü
|Õ°?SÚ;ç'K£?@Ö©A5?SÚ;ç'K£?ïïÖq˘?pÃÜZ ?`)Ž4gò¢?pÃÜZ¥?ïÕÝßÜöI?^¼÷rç?u"Úß?^¼÷rå4FGL J1033.1+4115?ºª™;Øq%@M0){úLbÀ9ÖÃƓÎÀ<T²¡¨[Ô@¼®Ç~.@¢Ÿ§Ñ?£Û1ƒIÛ?¤ÚT¼ÅÄ?û¹St[@Úº±AV?×6
G¿àĽÛB[¿çŠèáÖIM¿â±ªÂ‹Ö8¿ëÁ+Cz©¿ïùá½õ™uAGNfsrq3FGL J1033.2+4116S4 1030+41?ïû$¦[D?:NM"]?Coµf'î3?:NM"`?ïû`òv:?SÿœåL@?B|6'ù?SÿœåL?û?ï͆w×l"?xѪv³b?y<ÄI¶Ž?xѪv³b?ïøH*U'?C|icÐ?NßUÊ«_û?C|ic×4FGL J1033.5-5035?à¿Z/<S@×ÙõÀ9¦œë]±ŒÀ;êÅ®ËZ@ Ü:Óær?ù4m)Ï?»t#ùYs?ÉŒv›gÐ@¸Íi@Yùb¼c¿èõµ>:Î2¿Ûª7áî?µÖãÑ÷,¿Ï¢ô¡¨î¿âÏW xEŒ¿âAºÃ.¾AGNbcu3FGL J1033.4-50352MASS J10333216-5035287?é$WrÑ՟?Þàæµ5–?Ën¢4¸©'?Þàæµ5–?î
iŸ¨Ä
?¾Ôwæ-oü?¯)fs¿u?¾Ôwæ-oü?êÊ|÷V?°atÞ³ÿ`?Ç»"Ö"§?°atÞ³ÿ_?ìðxäre'?‰šTے®?¸|8ÜlÓî?‰šTے­4FGL J1033.5+4221?ë['N­µ@M{À;×`RP.ìÀ=qZ¶.ü@!gضea?ô6%UúÞX?ç`^*WÂ?ÙzH0yÿ?òµ
œ;5@Žî
å÷¿ë}Õ]¿ù«¿çÄ£2Ÿ¿ì	ۂr?ÌêžÚK:'¿Å±ÓLBβ¿î÷#"úAGNbllGB6 J1033+4222?ïù€ÚßOG?P¹T
%r'?Iü"'Âã?P¹T
%r'?ïýmS4å ?L¸Ÿ2†7ñ?4•fXÓ!?L¸Ÿ2†7þ?ﻏ¯Æ\?€Ë¤â°	?>Ühã?€Ë¤â°?ïý¸çaV?-Œ†!r´Ø?2;ÄõO¤?-Œ†!r´¼4FGL J1033.7+3708¿ïE]Îܪ@M¯Ž!–R½À:PêÔÑÀ<H™—ZÛ@»r‡[ÿ@bcQÞïå?®ì¿Uڗ¿±_2µ@3=¯÷¥@™£½‰ä¿Ý~7þÉõ¿éSFc'ŸÐ¿æȬŒ%=¿á¿ž{«¿Õ'‹Ã˜¾¿åTܛvékAGNbcuRX J1033.8+3708?ïõ])/4?R€Ée´'?UE­ å™?R€Ée´…?ïûð‹È?RMçì0ï4?@=Ó«ìÞ¿?RMçì0ï1?ïÓõJ`ü?z˜–¶F'?v@Zρñ?z˜–¶FŒ?ï¿-^Æ?pàïГ?€?ô¨|Îj?pàïБ4FGL J1033.9+6050¿ïÁ«ã›|a@HŽé_ªŠƒÀ7åŸËmÀ;B`	UX@?6̛@ÚÝ0È?›'Z¦®?¸ÈºI½c@ g»/ìVÖ@æ­Øë¿¿Ñâb
a-¿Û'Ã'ë¿âøÎ}¦ôÌ¿ã[+硺¿æ~±='ˆ¿ë‹µ±÷	AGNFSRQ3FGL J1033.8+6051S4 1030+61?ïî°ìª?^ 2ŠŸ©?aìOíU?^ 2ŠŸ²?ïÝû_É<?…9/Œ)#œ?qpÐa ?…9/Œ)#œ?ï\l?wE?—ùb¾Ý?"rx'Œ?—ùb¾Ü?ïÐë?mþ[NzCÆ?wò
wróÙ?mþ[NzCÈ4FGL J1034.0-2547¿ã[­jDÒ°@;—s}¦À:å
55lÀ<[€¼S@P³`•'@úњ'ç?Ð?Ÿ}3\y?º4v͒?íA".ÎI¥@¡6Æ愿ìo—!Å!³?ïü4Ï¥©¿èÞ¿¾qjQ¿Õià»[¿ïÿÙiÍy¿ïù¯æ9AGNbcuPMN J1033-2544?ïþƒ¦N?4ƒ"".>?/Ş‹$ä?4ƒ"".>
?ïúØHjn?aÍ
Õ·?DžßŽVF?aÍ
Õ¾?ï‰F¨è¯Ù?‰6½mÐÊf?®UÅÔ	¹?‰6½mÐÊh?ïϪ4B?màÊp2oÓ?x*åóÞóŽ?màÊp2oÔ4FGL J1035.1-0608¿Ì'ò)ÐSu@E•BB…À;$=Ìê)À<m"[tšÝ@yb|¡ç@cÄ*fÛ×?ƟEÀ~ŠÊ¿…T<S~"j?»3
nmñË@–Ÿ«Ÿ7¿ïÿDN
ª
?ïû—P=Ê¿ê$½Nª‡þ¿ä†ñ i,¿Ûèù¾_!¿ïÿ§ëkôEAGNbcuNVSS J103503-061204?ïóÉå#:2?^Øz­Ëy½?Xl5¹‹|?^Øz­ËyÄ?ïú¼ïð?q@€˜?E°@>>?q@€˜?îÒ•§?™|®Œ¼#c?¢ß¥Ž¯¸?™|®Œ¼#_?ïì3š'¢Ì?W—€'D5®?cÌeØ]3ö?W—€'D5¼4FGL J1035.3-2050?߁à–Cé@?ÎA=·ñsÀ:Õ%¹Íì‡À<'ã'÷Ó@ø'ֈ¸@Á`Dä5Ÿ?ƌÇÀ'?¤>"cì'u?ß±cÚðÑå@ ª'¹V¿Ñí¼Øc¿êo4 ñ|¯¿àµ[–ÿ‹¿àæ €~®¿ègMoœ¿ïúÒ~½uAAGNbcu2MASS J10351532-2050261?ïùÓ"[ª?FŠÄl{/9?H³±®'\?FŠÄl{/B?ïþy¨?/3?E˜üF²¢?(e|
èº?E˜üF²¢?ïãÄjS<?sSÃêsp?l;镬Â÷?sSÃêsr?ïó•Æ
9?D¥Wj§?YúÔsåŽ#?D¥Wj¢4FGL J1035.3+5541¿ïÉ¢ÐÞ3@J4…]¢r†À:ÁœiW²nÀ<¤tæY@@ß-Ím²@-î4üa?Àqç£è§õ¿dÄòÅZ?¦ŠøŸ—3?ö±
Ô~ó?îM¹kzw¿æä£î‡1¸¿è,ðùÒ¿¿á€ðя¿ïÿ³^¼£à?ïò˜Ù€9vAGNbcu3FGL J1035.2+5545GB6 J1035+5542?ïÛ¾"ª¦¶?w=²sÿÈ?r ½ª¬¤¿?w=²sÿÇ?îö òãŸ?±½—{'×D? ŸÝðÑÆ#?±½—{'×D?ï)—<À?"v«¦Lž{?šÍ|oÇí?"v«¦Lž~?îMÐe"1A?¡çÔ°Aò?«"ù­Üëî?¡çÔ°Aò4FGL J1035.6+4409¿äf=WÖC@Lö¸–ž=À:ó­FÈBÀ<É	<¿¤@¾_°i¿·@1"œâú6?Á¾'cò¿eBØYØ?p?¡WÝ´>6?ø¥b¥?î©?~ðöοׅ–AöD•¿è¹ƒäün{¿äùAj-›D¿Ù°}ãۇ¿í€·_þsAGNbll7C 1032+4424?ïҜx'?r²û8Ñ?v±Ã·pw¼?r²û8Ñ?ïÞ…èTe?‡g>?{ç?pü½ÕÍû?‡g>?{å?ï))ÍZH?'¨èoÒ?šÜÆT·
?'¨èoÍ?ï%øꞟ?òKƒ)?›@â¬,‰?òKƒ+4FGL J1036.2+2202?Ö4DþÙß@Mw™ÅXdÀ9ãíät‰?À<oîŒ:5†@Níd	K@¾€£ÿN)?³çØýî¾ö?©ëÿ~6"?ðüÛñ¨N@J‰)4?ɶ˜ØÔ¿çL?ÿIvÁ¿ç¯9>/H¿å'^!†ú¿ïÿ΢	?ïú²œ™AGNfsrqOL 256?ïþÅgçô? VjKwq?#¯é€¹M? VjKwqÇ?ïýp?P!Ú¤
£?74{÷÷æM?P!Ú¤
'?ïÝr¿:)7?rÉ·¾,?qF bëdU?rÉ·¾)?ïþº?ä¤?JÌÅøx¨?$\¡µ¸Ë?JÌÅøy<4FGL J1036.5+1231?™£û—@KŸ8ÅCkÀ;M♽«ÈÀ<È°­²UR@ ¯pÆf¬?ù ÛýÂ8?ßËlåÜhK?Ø6Ξ31[?üäª9$
ü?ôýìðƒ¶?èy¯†ßƒ¿Þ·";8?¿â¼g#û‡Ë¿ÁJùùUÁӿ煿ý±q'¿ï÷²ß:ãAGNbllTXS 1034+128?ï×qÞø«?t/5Ž'ª?tG{ƒ«C?t/5Ž'«?î—4Мÿ"?·êžÕ`B8?¦Œ²ö0
è?·êžÕ`B8?ï2à›>?"ÉsqŽ?œY£ì˜0?"ÉsqŽ?é´vÞçWÈ?®"ž`dÄÔ?É.$"b â?®"ž`dÄÔ4FGL J1036.6-3741?áFÁ-í@1äëÝ3L^À:ËƳ®ÖÀ<l$Ý/ @×è
Qé@½Ðæ7?у,$¡?Þ|7ž|ØC@Ó>ÿP3@§çC?¿©¶²"!7]¿Öš$‡¿ê¿>™Ä¿ì[1^Ƕ¿ïå¹,Ü×Ý¿äU?ÓªAGNfsrq3FGL J1037.4-3742PKS 1034-374?îí"Ó…é?©‹£ÆÐÓ¡?¡&²Î·¡h?©‹£ÆÐÓ¡?êÞë<ùº?ÈMo&®G[?ĄSÒ?ÈMo&®G[?í"a§R;?¡øæ¡àê~?·¦ìòÅn#?¡øæ¡àê€?ì@'?¡Å¨üÏ`£?¿ŸÕûo€?¡Å¨üÏ`£4FGL J1037.0-1954?æ;É]?›@@g¿rq6¤À;‡p'°H2À<¶žõ#-,@ '÷øt›]@hwhiÏ?ÊØï…忘~º£³¦?ÑM>!MØ{?ù£²½'È?éµ8%á;¿Ø×Bœ‡µ–¿éÞ@\ça¤¿Æ·¿^û
'¿é [À7?Ý¥ãߍï—AGNbcu1RXS J103657.5-195432?ïÞ½»i?p.rIŠ?p¡"~Kq@?p.rI?ïÀœ\	1Š?fò‹í¼?±Ñûg;a?fò‹í¼?ïžðùU:?…ÿ3Önˆ?ˆCÁ¹*±^?…ÿ3Önˆ?ïšoó…‹?w Å)ž™?‰d<œþ?w Å)ž™4FGL J1037.4-2933?æHK¢¼@8ß ù	kºÀ9º°"rÐÀ<MÝÙe@B†øXñ@0X<×÷£?¶4J4'æ?¤$§Õ?ì4"'òÜ+@äÁp‹?î<S£C^¿åiŸš´¿æ<m8è~Ú¿à»JùùU¿èŸó»NH¿êþøcSŒoAGNfsrq3FGL J1037.0-2934PKS 1034-293?ïõ‡qõî?O'ɨ?TñÓ"?O'ɤ?ïýËíÜõe?M…j™"î?1 'TÞ?M…j™"ñ?ïß¿Šz?l=ÀÚ!+1?p ~:Â÷?l=ÀÚ!+?ïøQÃÉ4~?:˅)'a?N¸ðÛ.?:˅)'g4FGL J1037.7-2822?ï¢ìÏßã@9äÚ<!~À8½ÔZ_ÇçÀ;°uÝÒ®Ž@4Ӕè@;7ÿJÎZ?¤[ã>?¸5™ióä"@oÄÖ^F@´·Ã{?¿ß3"À¼ž+¿á‹k~(Nÿ¿æn,Ε#é¿æ³¢.hž¿êx±ŒÕeù¿àšŠ?‰'ËAGNfsrq3FGL J1037.5-2821PKS B1035-281?ïûwõT™o?9ì§c‡Ÿ:?B *­šE?9ì§c‡Ÿ_?ïú^-¨ ?]Š6á?F‡I_©Û?]Š6á?ï^22n!ß?Äۋ1Ï1?"9¹²;Ä?Äۋ1Ï/?ïüÇž?-ÿÜô'ÂÐ?9Ǐ¿Cq?-ÿÜô'ÃG4FGL J1037.7+5711?ᨣZJÂ@Iäh3Æ*À8óz¶ƒÀ;s¦#×þ@ψ¾Õé?ü 
¡©2"?›
ß"(¹?²n+Â%©Þ@MÙ<FØ,@ rIs'r?îø^ õ-"¿ÓÕ-¤(ï¿Üw®F¥¿ÙpÜÁ·oî¿Ý{C&E¿å½•!dԖAGNbll3FGL J1037.5+5711GB6 J1037+5711?ïü¤Öýhn?6"KKã2?:ÙH¼•|?6"KKã?ïãÜ.' ?ŠžÏ:?l#Ñ}ìÞì?ŠžÏ:?ïØ-»^£l?{ÿbÁÊLû?sé"P®JY?{ÿbÁÊLþ?ï¹7–Heš?kXožå·?²mæ™
?kXožå·w4FGL J1038.2-2425¿âô!Š¾ ‰@=BDËáëÀ:Ž¼ôµ4À<dêúµ=d@^ou®­Ó@E$Ý/?¿á•¦'`¿žó/{Ý_Ü?ÞbyœÏ3@4J5Ù*Ô¿ÏΧBy¢-¿ç nºu\¿âŒŒÀÃ)5¿ã ¸§{Úl¿åšŸ˜·¿ïûxçrjAGNbcu3FGL J1038.0-2425NVSS J103824-242355?ïü·Šc?3uüé9M?:C«ôçsg?3uüé9MG?ïþq7þèz?E×ø¦Ša\?(ì€x[7?E×ø¦Šad?ï疘O?mæ'õŠðP?hig÷û°¢?mæ'õŠðK?ïýPPgv?$@jðñSj?5}|ÄK¬?$@jðñSj4FGL J1038.5+3926¿ÔPœ ÛÁ@Më¦ZÀ;Â:£À<éD=F²l@%¹r@¯;Ý%àd?͎àÃy¼Ú?²–ŸOwH?æ(ä$Ø&@Q-mÌaB?ïý÷Cõ"?ëg™6Jÿ¿æ9¸RÂD´¿áuú"pmP¿ïÿõEq#?ïÿ""ÆAGNbllNVSS J103845+392736?ïÿO……?(ÂE²…"Ç?VO^ì?(ÂE²…"£?ïûµô}ýë?]¾èÏz€ð?A(.X?]¾èÏz€ñ?ïneÁ`àM?ŽÇWŶ?'3GÓãöX?ŽÇWŶ?ïéì+.Ô?\?ƽj?fÿÔÑ+Ï?\?ƽb4FGL J1038.8-5312?áOh‹j@ž!S6Þ¹À8à@
²
ªÀ;<ý7Σg@j ñ@¿,0	³?³Åé?ˆâ?ÂMŒ¥ÀC}@¾ó
N7›@VÌ=…Ç€¿ÙXVñ?¿Üôï#¿èçóߋ@e¿ëfL€S¿ïý—¥£"¿à&OÀ1³×AGNfsrq3FGL J1038.9-5311MRC 1036-529?ïúÁü÷[Ø?FÀ~7C…?Dø"¡ß?FÀ~7C¿?ïö'ý…÷Ê?ls%#Øq/?Rúôk¬?ls%#Øq2?îorêˆ?Êâ}.V?¯¹ÑW}?Êâ}.V?ïÿÁ÷4£õ>÷GiÎ'¨t>ÿe®kå>÷GiÎ'©/4FGL J1039.2-2848?çУýkd@9¹:'£À:Ý¢'vgÀ<5ZŠ[@ G5««@XE ›€ú?ǘÓv	F¦¿ƒXÄx{£?¹'FÀÙ¤w?åЏ"Ýó¿å›°å"?ïUG$¿ˆ¿çРa3÷~¿ãÃ?ñBοÝJSá)¿ËòEžÅ¨AGNbcuNVSS J103921-285009?ïåãZ§E6?p8²!¥m?j¥XºÊ"?p8²!¥m?폈~–ÿ'?Á¾³ûƒ?³ƒ¼Hr?Á¾³ûƒ?ï‹Ď?ŠÜ]ëvÿ÷?>»~NÜ=?ŠÜ]ëvÿö?é½MΈtd?²

íÕH?É
ÈÅÞ.n?²

íÕH4FGL J1039.6+0535¿ìÀ²ÐÑî@Iüj%™íÀ;(D9P"À<‹RË~îó@!È¿¡ëù?ÿ(¥ߙX?Ä‹ªà¿¿¬ÄŒü*S?élIŸ†B¥?ùð3§!lŒ¿êF~3⅜¿êIEßaô¿åÎ	Bžá¿ØYɟñ¢o¿ÚKXC
ñ¿À|•|ÔfõAGNbcuNVSS J103940+053608?ïþ $÷4?&NÕalÓ·?-ý°†,¼;?&NÕalÓû?ïí13Ÿ
u?"ŒvÖÖ)?bÎÌ`õŠ¡?"ŒvÖÖ'?ïóœ AË9?dëDPûB~?XÇ¿|iŒ½?dëDPûB"?ï"0+ä'Ï?}r¶]"0[?‹3õÛL2?}r¶]"0Z4FGL J1039.9+7326¿íK…æHˆŠ@DF~RvŠÀ:ÕüÍE˜'À<Œ>õßÎ@€®É"¾@µý}nÁ?ÄHGAˆ
¦?¦ý&Ô!¢?Ǥõ'Î{ù@W¹‹Ò[­?ïÿý²Gæ¿è7Æ´{G¿ç7"DZ£¿âÿ¤àõx¾¿ÝÀ‡å</[¿ç<V]çAGNbcu3FGL J1039.5+7324GB6 J1039+7326?ïþóú×!~?ڑê»\? ÀRèý?ڑê»V?ïþÍɹs¼?BºÏ'€Ø?##dhÄJž?BºÏ'€Ø?ïõÊõ¦N?aFÕ}	}?Uôj³dæ?aFÕ}	y?ïùðïÄ?9¬ã55Ò¢?KÇÌ<@õT?9¬ã55Ò§4FGL J1040.5+0617¿Ü'ÀâoÏ@JK¼'cÀ8®ìúi¾
À;éOâ–b­@'gÍï@ߢºª‹Y?¡­&ê$¡u?–¬þG»wÝ?ò'b`Ght@ЀÁÜXÜ?ïš	`ÑÑï¿âsù+Ðhc¿åf®à¨¡Ê¿ãùÓá>ó¿ä` Áìt¿îv¼àE¥|AGNbll3FGL J1040.4+0615GB6 J1040+0617?ïûãiÛz?7p²[Þ?@r[´'\?7p²[Þ5?ïü?(É®?Qg'zšþz?>¹²£o?Qg'zšþu?ïÖ,óó?yt…ÛZ˜ÿ?té†vü…¬?yt…ÛZ˜þ?ïýRºåJ<?*Š¤B›"?5j(Õ®?*Š¤B›4FGL J1041.0+1342¿å¯
ÞåÓ@LcZ…‡"ÞÀ:åA—z©À<'šÎLÿ@ æã'áït?ùj;rœÕŽ?ÏSƒµ¬ ?Í2›ˆ²¼?þªYö›s?ÿT<xl·¿íO˜ß_vˆ¿ÖìaÝÀþ¿äCŒ?Å(ggÃ2Å¿çDÊ•Œo¿Ûdçî'CAGNbll3FGL J1040.8+13421RXS J104057.7+134216?ïñß?r?TÈëoñ·¾?\ÅæA—?TÈëoñ·Å?ïòàN?uvÙzÇHÈ?[üyð¿a©?uvÙzÇHÉ?…±>Œ?†/߼Ѣ?ŒšÞ"°\Ý?†/߼ѣ?ï0ò:>á?‡""&šL?™á¼x¸#æ?‡""&šM4FGL J1041.1-1201¿á¯ºÅ<@CÖî<³åÀ:Û·ìj÷ÆÀ<'á>sÙ@l^iAâù@‹QzF<?•5[×l8¿•õ¦4݂R?ӔÍí^<Ì@}禺¿?ïþòNf•`¿æ°ï@ëÁ¿ãøɪÙ\þ¿ÞBÀÄÖ´¿å/{]™c>¿ÄZÍÖâû7AGNbcu3FGL J1040.9-1205NVSS J104108-120332?ïü³3{€?3ùIËêæ?:g6d$Y?3ùIËêå?ïü<Ð~|D?aK¢ßGÎ`?>|æ^?aK¢ßGÎ\?ïñn
h-ñ?c I'aâ?]#å/¤?c I'aâ.?ïå~æÚÁ?SMåzâ|ô?jà%?²?SMåzâ|ô4FGL J1041.3-6437?ë²£~ñÒÀ¸"~–À:FU-XÿÀ;É'§
öc@æE'ƒ@U0 Y;Û?̉WW)Ýt?Í(˜zŠ¶@.QYŽç@Gì.'ãÃ?álÝÿ$7î¿ëz¥î;²^¿ÜN?=­Š'¿è©]&KÄ$¿èŒM€¼S¿ïÿøsCÄ{AGNbcuAT20G J104117-643103?ﬤáæ‡@?"'3}ñÐ?"Ödž^0-?"'3}ñÒ?ï÷fÊRŸ?iYT7ªÙ?Q3âkZÃ?iYT7ªÐ?í…Ý…b?¥&cèß5ï?·ÑÔëï?¥&cèß5î?ïQOo$>
?€ÐÓ­ªÅ[?•Öx>Ÿ?€ÐÓ­ªÅZ4FGL J1041.7+3902?œOruE}@NEž:WëÀ;&¹f¾zúÀ<í¬v0@ –$d
q?úµE\*£B?ÌEB;å?ÌHäu_þm@ˆô'@–Ó–•ƒ?í0G@0q¸¿á<Ybþä¿Üï|ÚÇm¿ÁvÀ{°¥¿åÎUÎh®?¿Ö² c¢¼®AGNbll3FGL J1041.8+3901B3 1038+392?ïú¸Âµ?@xŠ/•¤?Eè÷í4C?@xŠ/•?ïü5VJW?TÛ,¦ÞÁ??ÎUM­9¦?TÛ,¦ÞË?ïNjÙ)ù?}®Ê`ãK^?|:wk?}®Ê`ãKZ?ï¶×³»42?j¥ä
Ô#0?'J2ó"?j¥ä
Ô#94FGL J1041.9-0557¿ïTSa²ëz@F95" ¼8À:}ïunA&À<tރ®uÊ@ C?F'ß¼@y—=žÇ?µ]ÉòíÉ¿°Þ-mÉÝ?üTDZ±?ýƼT¯"½?ïþþ๿èL[B›Ûé¿ãÑ/"‡•¿àqýƔϿÜiµ©yŒ¿½¿¨L÷?AGNbll3FGL J1042.0-0557PMN J1042-0558?ïõ{Ýï±°?U\XÁBº?UD œ¢?U\XÁB³?ï´ìÙVO5?™ìæìå¬?'Äɪl2£?™ìæìå­?ïÚ )"À?t]˜jv?r¯ë=À»?t]˜jv?î
‰ÔÇß?–óØ*c.š?®Wb³'?–óØ*c.˜4FGL J1042.1-4128¿ØZÈ«S@.Pð"aùðÀ:×Ûô‡ýÀ<u]9—@ Îvúmˆ?û38Vˆ¢Ñ?ÅÈqÞ¿"~?Ïm¿$˜'@È\$Ä?þÄ·ÕnݿՁ¤k.Í?ŽP:¿Õ¨#>ߏ¿ÀÃ*Œ›"U¿á¬!±€–¿èT5vÚQñAGNbll3FGL J1042.1-41261RXS J104204.1-412936?íi Níš?¯¬Þ]z"?´¶ýˆ",?¯¬Þ]z"?ì—鈼Ê?Ç`jcß?»G ³º±?Ç`jcà?ìÚÄp²ü¶?§ø¥Kä.j?¹)Üzh[?§ø¥Kä.i?耇íܹ*?¬ÉôªQÖº?ÍýàHZ?¬ÉôªQÖ¹4FGL J1042.9+0054¿îÀ+Ab@HÄ$¢v·íÀ:½°}á­/À<qÈAíá@!º˜AÕ¸?ûÀ…`ýpÚ?ÄÍM¦&ð?­orÿ{ö›?étÀœ<â	@½±@Õ2¿ãЯgÏG¿Þå8Ô\ä¿Ý´	½#ã¿ÙyFÄܾ¿ÖÅl†;¿ÝÿePfËAGNbcuRBS 0895?ïüägOÛ%?3{"ø(ïA?8ÜŁ&Ûð?3{"ø(ï?ïý•JËM'?HŸ6`Ž¯?3U©¥–Ë?HŸ6`Ž®ú?ïëœÍ7a<?s€ArB|?dc2Ȟ£?s€ArBo?ïæý¶r!B?W—z×öWÁ?iIÞÀ?W—z×öWÌ4FGL J1043.2+2408¿ÝD»ð9Ÿ@NƒCc,CÀ9e"7ÉÀ<EÞ)ìb"@½×f"@_åÏÓ?¬6ÂZOy?ªÛ½ç'Ý?ú"Ô%†¢F@¬m™‹Ô¿Þh_ž¡¿àB1Ó·¢™¿åWøyùÁ"¿äÄÔævÁþ¿æ[¹™ê!q¿å÷]š
_AGNfsrq3FGL J1043.1+2407B2 1040+24A?ïù+ÍJÖ?K†[ö8£?KPÊ×ЫÄ?K†[ö8Ÿ?ïúñÂ:À"?[žÌÇ
6?D8÷ý¬í?[žÌÇ
-?ïäXfÌ)?p¿¨ãÒ>í?k§™3ÖðŠ?p¿¨ãÒ>ò?ïîèB†?RJ(o?añp½z>?RJ(o4FGL J1043.6+0654¿ÙZ@F'¤…@JÆБ}kfÀ;CT¸¾øÏÀ<¤lõÌ @ `Áïy&@#gÁLf?ÍBœGHéÔ?}ó0e7?²9Ž‰@?ÿižª%¿¹aǛ4¤L¿äPpZÛï¿éz¿8åz¿Ì¾MØü¿åb'q	¿¼öLWFŽAGNbllNVSS J104323+065307?ïùXƒ°f
?Hx…"¸?Jñ>gÐ]?Hx…"¸?ïúÀô)¼>?nê®,É?Dü/YU?nê®,Ã?ïò9Ìïò…?`AÁ:}-?[Œf öq?`AÁ:}.?ï݉oÖß*?\VãaþÇç?q;HkK?\VãaþÇê4FGL J1044.6+8053¿ïîÞøлG@A`»ÛãÁÀ9hùi
	ÔÀ;¶˜–dZó@ÓÕ)½"@'pOô4?²Ìx±—'?˼¤¡4™@'ÁC+λ@Ö»$,/¿±@}sž2¿ä(>ãjž¿ê×ÑÍmÜ¿ío±"‹c¿ïý"¶
+¿ï¤ÀßXÀ‹AGNfsrq3FGL J1044.4+8058S5 1039+81?íwrëÀ…g?¸;²Á§?´Dh¡ûÔ¾?¸;²Á§?è?̀e,?ÓàN}»çO?ÏßÍþkN?ÓàN}»çO?ê§ÖZÿ6?±=¬wí?Å`¦"›,?±=¬wí?䝹UÜî?¶+ˆ™i?ÖčTF#Ì?¶+ˆ™j4FGL J1045.3+2751¿ï²eî‡Ü@O
ÈuO7vÀ;<îM®ßÀ<¾TbWãí@ ÉýˆnU?ý÷¿¿ž!?ÅùcX¿ß©?o"=Äb™H?¨ÎI¾SÑþ@þߨF°"¿ïXPŽÌÝ?ïø]¿xÑM¿æ	°Š`A¿Û9ä<Õô>¿ÙiÝ^•a§¿ØÀäa>yAGNbllNVSS J104516+275136?ïÿ`œ£<?Ì2ô'!g?3ìk˜œ?Ì2ô' á?ïýü²=
ù?Bé9	]ÔÎ?0n¨0Z?Bé9	]ÔÅ?ïíÀ!Ì4?m/4Àê·}?b?Þà3Ëñ?m/4Àê·z?ïùtᔑ¿??>ʈÜ1Æ?J,y­¹Ö??>ʈÜ1¹4FGL J1045.8-2928¿éKS·âT£@9éã%Ô¦À9ù=¾§pÀ<?
›dtõ@…|Þwïü@ý.^¸<?¹ýjúIݚ?¶™_·ö|?ú¥)ð"R@uÏCtžã?J¼¼´¿æl¸ N¿è	ò&ùi
¿ã!ý•Âu¿ïÿù_|è3?à
 ÒH7AGNfsrq3FGL J1045.7-2926PKS B1043-291?ïý‡—ǯB?6VÛ:§xL?3ÃA…ô¸?6VÛ:§xp?ïþDG'•d?@ƒZ¸×*c?+»‡Ö©À^?@ƒZ¸×*k?ïÏ,ÛQs±?xd^£?xi'WF&é?xd^?ïÿPâNþõ?*@7KW?㶠!YP?*@7K4FGL J1045.9-2331?ߝN'H@>úÓØYÈÉÀ:ãHÇïî:À<'âÐDP'@ðëzŒãÿ?ÿ.˜I7w?ÚÏyº×?×¹ügÅ?ý)–·g	ú@isyIm?ïÿˆ@«Áº¿èÑ–8W¿ÔâÜʶ¿êáôÃIk¿ç2Àç¼<\¿ïÿõž}.)AGNbcu3FGL J1045.5-2335NVSS J104603-232855?ïÿý˜£?&‡D?@\ìëÀ?&‡9?ïüŠaZ[?V°0Œcöa?;¯¤õ-#ä?V°0Œcöi?îÊmNo"q?—*͖îk??£Y+
Øç?—*͖îk??ï£Æ²HÚÌ?qôĵl·.?‡SmÉLö?qôĵl·/4FGL J1046.0+5448¿ïAÇ}ÿLý@Kǟfb5À;;u¨ùˆíÀ<ԆðI©—@#·&rZ@u砍©¡?ƝÁ¿@"…4õ?ˆõŸeÉÆ?ún5ZTà,?î'l^YR¿éŠ¼A9[@¿åäÌh"ÿ	¿è¤8>4îõ¿ÉúÙh<¿ïÿÿ&¦³AGNbcu7C 1043+5505?ïøÉÇ´ˆm?MGź|ÚK?LØá-ÞLv?MGź|Ú"?ïöŒï'ßR?s‡õE~»y?Ræ ÜA]}?s‡õE~»u?ï—c@ÉÖm?';Ý»¼?Š'/͊d‰?';Ý»¼?ï·ð*øÉ?u9ÍS:<Ò?'=õAÍÇ?u9ÍS:<Ò4FGL J1046.8-2534?í®Üøƒ!@=Y¦?šIÃÀ: ⴕžÀ<hHí¯›d@!V%–c.?ù½)Î/£?Èpà'ÒU?ʈÈ%ž:@hæŽ>ò"@7]kT¿éD,[Ø¿éýºÀÛ§Ü?͇ìH=o¿Ó—dá6¿Éø–T?È¿é"VœoAGNbll3FGL J1046.9-2531NVSS J104651-253547?ïç·»•,?d|±®+†;?hHDjÓqÜ?d|±®+†4?ïûå¿"².?[Žb¢´¢?@iu7JÇ?[Žb¢´¬?ï}"aêH	?ŽJÕ}M1?Os¶þÉ?ŽJÕ}M/?︥mŘ?qÞk€"±a?à¤Ž™Ã?qÞk€"±^4FGL J1047.2-5517¿ïí¢´óË~@+ $bµØÀ9Ÿj'E'À;]ûî"‡ê@u¤œ×è@'iߗª¬?Å­W¼w¯?§YÿáÞ=?ܕĢܹ@«ÙK=¿áÏ$Ã-è¿ç–¾¡¿å,¥3Ìá¿çŠü4µê¿ê$¼ãJ½"¿ïú
ÝÿzAGNbcuPMN J1047-5513?ïõ½ª´æ¡?UF­‡_‡u?T"ª–2¿B?UF­‡_‡^?ïò´h."˜?Œx¢÷ï?Z—/£ºÏŒ?Œx¢÷ï?ï"ëí*?–s"®ºì?Ÿ
b'NZÍ?–s"®ºë?ïú0®K¼?9Káo£ð5?G=FÓ¥
?9Káo£ðH4FGL J1047.7+7238¿î+qØÅБ@Dþ<Q‡À9òOƒËÑûÀ<H‡Þ†2µ@¶;ÁÍ@UYΨo?¼grUx?½Y''b?üR¬9¯N@ÍÉæhE?ª)'þþUä?ï_]"Y
¸¿áµ¹À€Ž0¿âö'î½b¿æ?)@k*¿ãþ±·!jAGNbll3FGL J1047.6+7240GB6 J1047+7238?ïø}ù¾^W?QˍÓဈ?N†¤z?QˍÓဋ?ïû«i}Ô<?Wš$^*í?ARZ¯
Ý?Wš$^*ã?ïÍšÉ?{•§k²»?yu2›r|µ?{•§k²Ä?ï냔{kh?W5e¡TÎÏ?d|k""™é?W5e¡TÎÑ4FGL J1047.8-6216?ïí»Q펊À*~#ûÀ8ŸüuÀ;$ї6èÊ@nâP3@2²|¿n??°ú¥Î\
?²—ºÇ<@Nõ üÐ@ª;£!¿Ì<Õ"oß¿áùbW
-¿çOÒ:Ê×)¿æáÑv¹¿åö8Öá"Å¿ïÿþ½à ¿AGNbcu3FGL J1047.8-6216PMN J1047-6217?ïýÔö"«2?3²«r¬áÃ?1XKÚ¦qö?3²«r¬áí?ïûŒ19.Ù?_å࣬S¯?AÏ;Dý?_å࣬S®?îí™À÷o?™¤8ã¬?¡&nóð‰?™¤8ã¬?ïÖæ·Ë7?b¨RZ•c?tŒ¤ds?b¨RZ•g4FGL J1047.9+0055¿ßƶK2¡ì@I:ÀÛ'À:n©ö/yÀ<?µÚBV@@«6$)U@U`"¥?Ãá!¾Ð?©9½;	kd?à½2?î,™@'ûF²Â?ïÀRÀí ¿ç…Þz¿æÊjåQ¿ë°R®"½š¿Ã"úÉ4g¿ïÿ$m'MAGNbcuTXS 1045+011?ïýُȇ—?5‹Æ§âf&?13»ÃI'?5‹Æ§âeõ?ïý'\§?M8!rÛDÒ?7ÃuêÑw?M8!rÛDÞ?ïà‡'¡ÔM?n Â-åZ#?oxn^+³'?n Â-åZ&?ïòi1õxÁ?R¯)äàP?[-œÑ?R¯)äàY4FGL J1047.9-3738?àÜ^Ë®ë@3*ýڋÒÀ:ÛCîlYÅÀ<ˆU|3WE@!"':ûSž?û9JÚåª?Æ*ñÛ¥Ø?¹ûOìýD?öâý¹÷@îA~5»¿ïýš?[à|?ïáäVVMê¿ÛÚ胿¼ŸXö;¿âd.þ›&¿Ým ßôq×AGNbcu3FGL J1047.8-3737GALEXASC J104756.99-373730.1?ïþÆC$?-ètØèÃù?/ƒžËÍÒ-?-ètØèÃü?ïøN¾¦û?g³b{'ý?NÅ¥d?g³b{'û?ïîœSwAb?bÍy~¸üc?ac¬ˆ¾ŸE?bÍy~¸üi?ïºâåÐ"R?q7/4‡w?GF‹÷k)?q7/4‡x4FGL J1048.0-1912¿îÔÛ@ø&@Al½QðÀ:ùíp±CÀ<ƒCË0ëZ@†8sŽíï@ÞõfI
5?Ì}º•èŠ?À€È|)F?ñCâtÔ¾?û0£0œ*?ïÿì»"¿ÛÆDóO¿éÇ :ˆ¿ä/9ÿU5<¿ã¦ YžØ¿ïÿÿ" 5•AGNfsrqPKS 1045-18?ïùø=œ7f?M´ŒJ¤8?H	"e?M´ŒJ¤3?ïÀû˜öO? çCßÀ)3?ÁÂl¡? çCßÀ)3?îÚ×`oëð?•êGk_"x?¢R‰ùA?•êGk_"v?î
ò;—?=g]ߍh?¯Pß¼O¦š?=g]ߍh4FGL J1048.4+7143¿íûqº^ô@E$	_$RÆÀ7"
ƒÁÀ;4òtý@/öU²9#@ ;>šo'?ÈîN…QÂ?µÂ¡"~–@&0¼Y¸:@!áªqKµ¿ïÿÚáb†¿ê[y£Z¼?ïî.¡©¡?ۜ@]=Gß¿àLZK¥ñ¿É¢
cAïAGNFSRQ3FGL J1048.4+7144S5 1044+71?ï¬Ë*ô?·{Ï×»ú?"øM5BØ¿?·{Ï×»ú?ïâ1}aÂ?L%sVÊ?m~΂ž>ñ?L%sVÅ?î˜(ܨàº?ÝÅ;¦?¦}r5qôy?ÝÅ;¦?ïÿn•pïŠ?̲îüœC?-Qâ×U?̲îüœE4FGL J1049.5+1548¿äÎXGYoé@MÉrGE8ïÀ9ï`sÞ.À<_þ99@I6ù;jº@$ù´Œ?¹äÖÙÀü	?¶‡ÑßÊð?úd§՟Ú@V'+áÛ'¿ä­òˆH8¿äJúú¿àc^Caÿ¿ãmó=yÞ¿ê´RbM}¿ßä«üƊAGNbll3FGL J1049.7+1548GB6 J1049+1548?ïÑëÅt—™?u=o­‹0a?w
E´3F?u=o­‹0f?ïöªpæÌ«?i~HÁ™yh?R«2f©û?i~HÁ™yh?ïióÛ	M?1ì`ÖØ?'Áž"žÖb?1ì`ÖÙ?ï^'å"æ?rdëŽÞ?"/£\/c4?rdëŽÞ4FGL J1049.7+5011¿í¨§œ·¹&@L¨6m
JÀ:îÂfA}yÀ<Õ? §?u@圧k@ÂeŽÐ?É7ôãí$Ü?ΏH\æ
?þJ†_¡P@é¶H¦âØ?îrò yI¿ãÊ\º³¿àd¸aý–¿æMzV[V¿ëoýV'n?Åb¸ÜÕÙfAGNbllNVSS J104857+500943?ïØ4s抟?uFçmÀʙ?såÆº±?uFçmÀʖ?ïø×Oge?o_XÓgÀ?L¢ÂbkP?o_XÓgÃ?íç‡ê4'Ã?¡+Wıyô?°ÃÀ®[qâ?¡+Wıyõ?ï¨k$.« ?rMCÚ6TÕ?…å6ôUì?rMCÚ6TÓ4FGL J1049.8+1429¿²‰äÚöÉ@M'bS—WÀ9LwH5ù·À<2¾Ÿã_¶@q*EÎÁD@kÉÚª"?®žˆýÑ7Ò?²=ïN×Ôh@K¡F6E6@Ê
¥/$¿l{É:Ç¿ä«QݘL¿æ¯Õ`EK¿éœÀË6ʗ¿ð?ïþËÌÍAGNbcu3FGL J1049.8+1425MG1 J104945+1429?ïÿbz?ßč?­ÿpÏ?ßčÙ?ïúh½_¹8?\D}Y}&?F]
Á?\D}Y}3?ï¼Ù..@i?'´ ÌÈ?€É´toåã?'´ ÌÍ?ïö‡Æî!Y?G5»ÓÃLA?Rðr#½OÉ?G5»ÓÃLS4FGL J1050.1+0432?ëþ{'õQs@J¨Ü]cˆfÀ9UóU͒À<,	óžÉ@Yø6zæ@uƒž?°‡ÇŸ'UR?³óÛÚ[×?þœÃk$;@£3ž¿Ý%#:—«ƒ¿åâ1ž½d¿æwKüWÔÓ¿ê\ÞCÖ¿çŽR"_¿ïþ‹ Z›AGNfsrq3FGL J1050.4+0435MG1 J105009+0433?ïÿwªLu?
ióŽuF?
¶1€v?
ióŽuE??ïü¨{e9$?SÊÝÉi
>?:¼$Ö6ã?SÊÝÉi
3?ïÙ%÷§?qcHb¯À?sq|í+™?qcHb¯Â?ïÿ"í»fÕ?^®1ðç¯?đ&J®?^®1ðè4FGL J1051.2-6517¿Ê/1®l¡·À0¹~;oBÀ9l™ÝŒ7±À;·ÊX~F@"ýûÃÛ7@ÛØ{V¸s?´£è}ˆk?ªœ©!)£ñ?ô‹'æÎ×?ô
ôÀéú¿Ò.žÎ⧿Ö*èÁŸòú¿çм{Eñ|¿å¸/A8¿á¥Æ}þ2 ¿è"ó!uE§AGNbcu3FGL J1051.5-6517PKS 1049-650?ï>×;ï÷Þ?'š:P<ìù?˜%'7?'š:P<ìù?ì)êþ?Å|…;BPr?»–´¨U?Å|…;BPr?îAûi
R?›ÇÄrœ*?«àIn/Zê?›ÇÄrœ-?ähd©?µT½Sł§?×/õ7ÝÀ¬?µT½Sł§4FGL J1051.4-3139?½$ùœ`¢ä@8¡¢¤Û<À:žpÆ;¹À<OÚy]¹ï@ÿ·1Ô@LaÿÏ?Þ'_Tú-X?ïü«ë«µ@ BÛ@ í‹^B¿à‹ÛÀÛ|é¿æ(bÙ	¿ìÓ¤¢š¿è9ê™w5¿ÀÄbÛlwÍ¿àöÿ¦=ìËAGNfsrqPKS 1048-313?ïªòŽÚ?'$U4êZ?…C[Ü[É^?'$U4êZ?ç;µ£'Â?Ôÿ'|²?ш"¸Ýð}?Ôÿ'|²?ìÍÔKöh©?¤°/¦"–·?¹'] Lº¹?¤°/¦"–¸?æwµÛ»F?Æî@?Ó"Hˆår?Æî@4FGL J1051.4+3942¿èe±sJv@OS?B5/À:Ò ùtÌÀ<'Ejm\$@!&Ö>°!?ù•¸~a.ï?Ä®j·ù?¼x`äÇ??úa…Æ}þ@B·¼Dif?ï÷"ÁpME¿è!œÓ	ý°?ƐöGo€A¿ä‰6?W-ä?±Ú, ‹À¿Ú"þPÅAGNbll3FGL J1051.4+3941RBS 0909?ïÿ_|Ú±Ï?rÅucÂÓ?d©Æ?rÅucÃ?ïü0 œ§"?S^·}ˆ—k?>zûÃf.?S^·}ˆ—e?ïãFïBÖ¸?ufÔeŽ+ï?l¹½)HG?ufÔeŽ+í?ïô&Bàd?NMr]+¼'?W³z?Û77?NMr]+¼4FGL J1051.6+2109?×1Gޙ_@O
üçFÌÀ:Œ@O{hVÀ<Z)ôÆ@èåtc+?ýy*GÒ'?ÚÉLÅUŠ ?îâÁ*Øß@ã*!;¹ê@´ÏüØ`¿è³pÛ4n¿â.	È֞¿êqN õC¿ï£GÞ#¿ïLZUÕõ¿ënƒÁ@&·AGNfsrqOL 282?ïýkÅÁބ?Hs¿ŽKF?4¡ÑñÒM?Hs¿ŽKR?ïõ¼F£ÞÍ?vŽq §æ?T‡r¸Bbh?vŽq §ä?î(¡b2Èæ?›±æ*@?­uéÜÓqº?›±æ*<?ï½ÒáðàF?w{²mtz?€‹GƒÇî[?w{²mtz4FGL J1051.9+0103?ÛfÄg@I¢pÁ3;—À:¨ÓÚGóÀ<zµ'»@ "~/Zá?ûÔ¶:º2?Éž–Xœy?ÊÁG3@nÙ8@ Þò¿%¿î^&@Üi"¿Â'Š^h@0¿ÔHÀc1þ€¿¶[Ø}Z¿ì\'Á3¤?ÀÅ`‡TG«AGNbll3FGL J1051.8+0105NVSS J105151+010312?ïÎLO]Y?|®‡ôwé?xÙØQ~R"?|®‡ôwë?ïúi—€¡?Xߒ:…Ž?FY¡ý{Ñ+?Xߒ:…™?î,@"?žÌ ¢É?­;ÿN
ÞÆ?žÌ ¢É?ï¬ò·,÷O?uµC;ðÿ£?"ÃR4Â,=?uµC;ðÿ¢4FGL J1052.3+0818¿åáKŌ"@L.‹*kÀ;(Ï,"žÀ<€w˜½Ñ‡@éª{i,ê@‰$y\p?ÉÔ®ƒ
¶è?ŠÉ'"C
?¼"•£Àº@>%ühñ±?Á©p¨	¿éº¼"pdí¿Ù·áéÏ¿êÉÞÛÃ
¿Äpjá C'¿ïÜè‹+BAGNbcu3FGL J1052.0+08162MASX J10522451+0814095?ïü¼âä£+?8µá©¾F<?:èÚæÖ?8µá©¾F
?ïýÔåÚCF?KÒz-àH?1XÑ-åÍ\?KÒz-àL?ïÃ2çŽd?ßì6?~uæŒ8Íù?ßì7?ïý7öcþÕ?*Dž9Ú3?6@Là	Yý?*Dž9ÚÏ4FGL J1052.9-3743¿Ù/Ÿ° Q°@3r§›ºÜ
À:ŒPx¾W¿À<|ÏÓèJ@ U*Ï?ÿI¦Wíþ?Áå'Ác?°JCp?7?óec>"º@,ŽTÁù4?íº|CG}¿ÀßsXd¿äµ¿Ý…*¡¿,ü¿Ð?›PÔ¿ë.
ß¼"šAGNbll3FGL J1052.8-3741PMN J1053-3743?ïï¢JÞë?Z²­Ð.ê?`]êµ!Ú?Z²­Ð.õ?ïø²¤bæ?g°Œé&
?M5ntg©?g°Œé&?ïÝW|Û?u­';`LU?qvuTA'§?u­';`LP?ﻳ&¢®?jR' ×Ž?6~T5?jR' ×‹4FGL J1053.7+4930¿ïÿä#†í»@MEhÀ:´ñä´JÀ<m¶
éh@nˆcf?þ/}0­Fö?²ë¯α?žn"h¶?ìܲÞd#ì@.ø3
ò?' Wú?Ê
áÄÚ¿âd…†"¿Ýýc˜€À¿ä&@×`¥?º>¤@¼;AGNbll3FGL J1053.7+4929GB6 J1053+4930?ïýW`?/k[͆?7ÏõGdø5?/k[Ík?ïú%ye§­?Y¼éO7ú†?GjiaNM?Y¼éO7ú?ïæ®ϔ?t7¬Œ?iQø0kqá?t7¬Œ?ïÊ`F§'Æ?isAjP©†?zÏܬ7·?isAjP©Š4FGL J1053.9+8628?çÑà
@>0)à¤&À;7Žd²1@À<Œ†ÿc"@ =ºßd@W#"ú?ÆN­øvHÝ¿ˆGQ€Ù·Ê?Á<×xLm@(W$T9¿ïwWÂHå?í	ۂr¿ëx¤ Üš¿×ë'D"Wá¿Ï
W–꽤¿á#=Qš&‡AGNbcuWN B1046.1+8645?ïåÔ1IZ¢?iÎ5ÓÒ8?j+ζ¥_}?iÎ5ÓÒ7?ïûÆÆ‡Å?`là{GÁK?@äçÍàïø?`là{GÁH?ïÔ¤¹Û?v~–›ä?u­öù£3?v~–›å?ïëiu/D?WZÔtv'?d–äŠÐº«?WZÔtv'm4FGL J1054.2+3926¿ìp4c¹@O`ïܜM©À;Ê;"À<±ákÀB{@&a"ðh@h·¼šO¢?Ô	éã³ï?Ø*Ov`@ÇMœk2@J‰äDãŠ?ïì,CTéf?á£ÂýÁy¿â° ¬³R¿äiêIµU¸¿ïü`¾†¸ì¿é'kb#¶"AGNbcuCRATES J105433+392803?îºâóX
N?¢Nº–™'¹?¤QÐÊ+%?¢Nº–™'¹?ì—å|£ô¯?Ŏ	ÿU?»@ÔàZ?Ŏ	ÿU?ëø&³§1é?¦ä=ÌàË?Àe1c8X?¦ä=ÌàË
?ãõµ?˜kì?µûˆ¿Á?Ø•€Ï((?µûˆ¿Á4FGL J1054.5+2211¿ïf¹>ò†@O…" ä¶À9s€*]À<ò³ç#@,4XÍ@¼{ٕ2,?©?Ï£Á»¢?§S›2 ç?ü½CŠU@ÕàòŸ?ïû)×iß¿áón!EÊå¿â88 þ¿áI™;¥È|¿ä5D௭­¿äáü>ª_ºAGNbll3FGL J1054.5+221087GB 105148.6+222705?ïûÝHÉX¼?5­ûý—'Z?@ŠÜڝI?5­ûý—'K?ïø½9G¨›?d®³ƒèú
?Má]þ?d®³ƒèú?ïë}_'Xt?jFWèÔ?d' Ø§Šù?jFWèò?ﳈû¦?rÿË뜟?ƒ>ÿA"?rÿË뜟4FGL J1055.5-0125¿ë¥0^õõ¾@I
ÅÁ?ÐÐÀ:G­§m—³À<OÏôŸy­@ >è{~ü_?ÿ‡ÚTtÌ?º›äbÈ¿ŸZ|Î1Ñ´?ä¥	Œ³@@"¯Ò–¿Ãòæ&¨¿ëù@€¿ÇK	ÿ\–¿Þ|_p#¿áb¡ N>§¿½@Y6}©AGNbllRX J1055.5-0126?ïõúâÔë?HkóŸx´w?T
:V)ôL?HkóŸx´N?ïü_ô'ƒ?RÔH¾XX?=[kç?ƒ?RÔH¾XW?ïìñ[?rBO.nöM?cbè示?rBO.nöF?ïÏ·ó¨ñg?c'§Ïr?x$+‡Lž?c'§Ïv4FGL J1056.0+0253¿àT›
"'O@J£þ¬BêÀ;–(Ÿ~¶À<­¸6<Òï@#U´D•±-?÷UGZ1¥?Ð[j‰á•²?«™lÈ?Þ6B\Eü?ý¹U̐<?ë~·–ã?"(H7k?íjcì8¢ß?Ôìi ,°¸¿Ýê!;¹êr?Z9¡%BôAGNbllRX J1056.1+0252?ïý~Z¥à×?0@š_Ýà?4
*ÐùS?0@š_Ýç?ïú/™0lÜ?pÇ?‰Ùi¶?GA›>L?pÇ?‰Ùiº?ïêÊH(?mϨ&û?e5ä·×üD?mϨ&î?ïÏR…8‡#?nA@Bz›?xV½c¼o¨?nA@Bz—4FGL J1056.8+7012¿ä"ø|v˜+@EôÚ<÷À9,azn['À:§9zu$@TdhµK&@Y£ÙŽ|?¿¯Ý'ãɾ?½*Œªü@	Ì΢âa@ÑD]'""?ؗ,¢z¿áø"»ìª¹¿è³Œdþ¿èžaŸ­.ø¿ìa‡"à¿ïý¥ýÖ.AGNfsrq3FGL J1058.1+7010S5 1053+70?ïÉÏíá7E?}¾"LȐ?{	d^?}¾"LȐ?ïú¶!u"Ö?gˆ†Ä	X³?E'z)ì§?gˆ†Ä	X²?ìyÂÊË k?¨Ç&'Åݎ?¼1é©¢ü ?¨Ç&'Åݏ?ï÷qí€?E"¸pÅ?QÓà$ÿµ?E"¸pÍ4FGL J1057.2+5510?é?'ì/Gá@K"£½ßÊÀ;7='¨»À<á±¾SF@!-ÒK;é?óT5€ëM?ã9û¤P­?יG¤¯L^?û"üa'@˪ZÜð[¿íÂÎ{ùu¢?ä?°¿í#è§ô¦0?ÝWH…Ö¿Û'îM®ß¿êP
¤ž°ZAGNbcuSDSS J105707.47+551032.2?ïü""+‹?;NŸÏ×_	?;[f§£±?;NŸÏ×_?ïûesœ?aRSLÄ´Ž?Bj2ÚŽ?aRSLÄ´Š?˜"A?…IB¡Ž?‡Ùþ™Û/ƒ?…IB¡•?ïû¾e"ç?7_¢{ËÄ ?Ai­¼^ß?7_¢{ËÄ34FGL J1057.3-2341¿³1ö¡"@@ó.ZÀ9ã3cښìÀ<PÕ˨à@+³ß•ý-@SEø1Õ?»Ñá߃ˆ¶?ϙ‹Và·@r:½k/ú@Ü¥!âþ½¿ØHˆÚځ–¿Ú¬Cà‡¿äû…LXž¿é¼­?"¾¹¿é?#âqŽ¿ïÿס<%JAGNfsrq3FGL J1057.3-2341PKS B1054-234?ïºøæ}·á?€2{/@˜?AÆ`'Ê?€2{/@˜?ïð )…Š·?v=ðå§j?_¿¬ôêŽè?v=ðå§j?î¾=̪Š?•G4#
†?¤œ#5Wa?•G4#
…?ï!¬?ƒÁH'&?›Ðê}¾#?ƒÁH'$4FGL J1057.8-2754¿á)'N´@<•ŸÓo~=À9ùhG6‰À<BÃú–3´@ }'Ñ#I?ý"VÁ­´Ú?¸cfAR…´?®3Øþ?ö"æ™ýl¨@ WمÂÍ?ÑÀ&€ó/¿Þ=¡`¸Q–¿ß³þ4Måf¿ÒõJd¨ E¿æõ2F¤)@¿«ÀÀ9ÁAGNbll3FGL J1057.6-2754RX J1057.8-2753?ïüÕ@VGT?,S¬O2a?9UýMÅc?,S¬O2?ïý>Ù{×p?M:Û\Œý)?6	4!Ds×?M:Û\Œý8?ïïS/B¦_?qRºØžå?`¬Ð½Y Æ?qRºØžç?ïÖÆ…`H?\v¤2Yæ?tœø=OÜ&?\v¤2Yã4FGL J1058.0+4305?à‡?$ž"@O	V"À;Q4‡Ç	>À<ÔLR¾éµ@ÞÑrMû6@'¾´V?Áø­æ­ž‰¿«þym)N-?ê…¸Qì@	?Òñô¿ïãåÌÞÀ?ïÛ_W5¿é¦n£¿é~T>p©
¿bÜ­>‰u¿à¿Ýƒ(iAGNbllB3 1055+433?ïû9Ö¸¥]?KÖ¦…£6?C¥j‰"?KÖ¦…£/?ïü¢4`¨'?RôÞ¡I?:î\ú¾Æ¬?RôÞ¡I?ïzB*Vý×?Š¾+OÔÿh?·ºµ E/?Š¾+OÔÿh?ïýÀwL?)Øg¯h?1ÿœG}©S?)Øg¯hë4FGL J1058.4+0133?ïqãÎã@JbëÝ3L^À7æR¯Ð=À;0;pïVe@À'D@…›"/Õ±?"rºÝŒ¾?¨¥ã»@'»=XP#@ÄaՈ¿ ªÆ©¿áw¾þX
¿ä'Þ^ð{S¿ã³'i#°¿åc(X䝤¿ç&ÆsxAGNBLL3FGL J1058.5+01334C +01.28?ïýͳÜJ?.:(Ɛ?1'aå·X?.:(ÆÇ?ïðÃ/²]P?u;z/8y›?^y ›E_?u;z/8yœ?ïÕZk*0–?{·¼í?uRÊjç´-?{·¼è?ïòpîÛ-ð?J'–Ž¤[â?["I¤!Ö?J'–Ž¤[×4FGL J1058.5+8115¿å.8ѓ@A_ d#–À9ÃÁ>#Q>À<¸Îé@'<ýâC'@÷¯~Þ,q?º °å¹±?Á¤Ÿ\&G?øQGñ0Yd@CäýÆö¿Þp*
ag¿æ5deÛ&¿æ€\a)惿äJ¯@ŸØM¿èæt¾˜×}¿ïóÓl#>ÉAGNfsrq3FGL J1058.4+8112S5 1053+81?ïî—ʠQ?aã†)<?a=h5_®?aã†)<
?ïýŸÖº0œ?KxQˆ?3J.{E?KxQ|?ï¿Ô÷U?€U^µn¡?€;øJÂ*†?€U^µn¡?ïü•ªêîÖ?.)J쁄?;R¨¨‰OD?.)Jìe4FGL J1058.6+2817¿ë}ú"l¼ @PCƒQX¸(À:%W¨]'À<vÄÀ§%@É{'G•Á@˜>{?´©8ÈôP?£×¡çñÁN?í²"\KZq@X¡C§¿ä|)±ª1—¿×ºÈ"W¿ä±õ桊)¿åñìa<°à¿â3͌æ-¿ä¥\{¬AGNbllGB6 J1058+2817?ïû'c›"?>¯Òsø*$?Cbq'ïþÚ?>¯Òsø*=?ïü•tîs?R(¾mË6i?;WDXŒcŒ?R(¾mË6d?ïâÔëà¨~?q³¼°Ž<b?m+W‡?q³¼°Ž<_?ïûªWŠE6?2D_;Ê0?AV¡Öë#T?2D_;Ê:4FGL J1058.6-8003¿ìßµ~;ÌdÀ2IêþæûLÀ8Òfàß©HÀ;ËûSÈÕ@<'UÓF@ö@×`¥?§Ã¾s?ÂÆ'De
@0¢_:ù@½r,mFT?áÀ½šTÕ¿Ðâî![Dt¿â֓ n¿ä‡âT1¿é|õSԓk¿ìð"rϏAGNbll3FGL J1058.5-8003PKS 1057-79?ïyD ø2?ñK²¼Vø?×n[àù"?ñK²¼Vø?ïíãâ(²?{—̸/}Œ?b€×MÎ?{—̸/}Ž?íK09À?¢Ò!Ã(ãv?³¦~7Š?¢Ò!Ã(ãu?ïó¤æ¢<_?Gá$,H?X¶2»‡B?Gá$,H4FGL J1058.6+5627?×!{»§…A@K7Y‰ßsÀ8+È5ŽWFÀ;‹ïXèÏb@B_ úa?ý¹"vD)û?šÀÜÿtê¹?§t®R¹5k@IÄ|œ2Ñ@§'ˆÛu¿Ð'¾^"¿Ür´þNúå¿ÝظG¿Ý…bÀi'¿âPÝèþÝ¿ÚbNAGNBLL3FGL J1058.6+5627TXS 1055+567?ïþ©8\ß?¼g	4Y?%nüz1ós?¼g	4!?ïùøЀN?ZŁå´?H½þÇ­¦?ZŁå²?ïÝ-ÄÉnó?u°õ'¼ý€?qi›H†ð?u°õ'¼ý"?ïý?ÌÎý[?$©Åsɇ?6™ˆ/d?$©ÅsÉ 4FGL J1059.2-1134?ï1ϚÒ±@EWçl‹C–À8*obŽj'À;ˆÅFƍî@0¿¿s@´ó\ƒŽ•?–Ä|=µ'?§*ò®~@
 "S.{>@#ùñÉ¿ÅžÚK:ö¿àˆbÚÀ«V¿âd["{L§¿á!Ä«–`¿å°pÀÝU[¿å7i=±;wAGNbll3FGL J1059.2-1133PKS B1056-113?ïþm
Œ?*'dM¿¶?/y/W>x	?*'dM¿š?ï÷fù-q\?k¸{ä?Q2
¥H>?k¸{à?ïßÜR¶µ?t
ëo
?pÖ¤¤ž?t
ëo?ïö³sÿD?BÐqݑQ™?R™ùx¹?BÐqݑQ¢4FGL J1059.5+2057?녗DÃà@Oâ»ìª¸¦À:"'Gm|ÛÀ<o¼Õ±@‡Ñðøü@-›ymª(?Â;Ñ&ù"?®h˜Å´)¾?äsmµæz@	œ²êx"K¿ßÏÙ\'HC¿åF,iëV%¿å´üÌnÙ¿ä'zޢ߿ï\tÜJï?æusê³g¡AGNfsrq3FGL J1059.9+2056MG2 J105938+2057?ïúÃL´ª?@Ëìí¹}/?Dó'Í-Z¹?@Ëìí¹},?ïý@£ ̈́?Kô=B!X'?5úæù"Õö?Kô=B!XA?ïßo&v«'?uÊG0€"?pHlĪ??uÊG0€"#?ïô^X³1?J~¾'«?WCN™Éž?J~¾'‹4FGL J1100.3+4020?ïàØˑe@@OÈ<hfÀ:7|ˆçš®À<i÷_GŽ@ géAørî?û…tH§8¿?¾ÏtòÆ0¦?¼ìæÞýÝ@øSÜ &ç@I¾ð–*¤?ïsy³J¿âëÈæà>½à ¿(¿ÕJí#¯\¤¿ÙXI"ç«¿å#傦8AGNbll3FGL J1100.5+4020RX J1100.3+4019?ïü®¾¿Ðï?9¶I"u‡?:Š
x‹?9¶I"ub?ïòTöÑð?r.s'½Ç?[V]È">?r.s'½Ç?ïÝ«yZ
ø?xŸõÖu0V?q*CRúƒ¥?xŸõÖu0W?îõÕ&Çó?†¾"–^4~? ¢­"€Ç?†¾"–^4~4FGL J1101.3+7017¿íñÖØg"ú@Fÿ¼ä!À:CÃz=³ÀÀ:ìL>œóÁ@ÁÿiW@6
éh?·©׉>¿»iˆúe@G£áñø@]˜oVпÓÈ^˽X¿èéQgÑ q¿è]Áa^¿©¿é"'Ž¿á;Tiä ¿â\‹áõþÊAGNbcuGB6 J1102+7019?ïæZ
î#?p£Í
³øš?i¥ûõÜÏ?p£Í
³ø™?ï®ÝÒ Þ:?¥­ÌÞofK?"H‹WÈq'?¥­ÌÞofK?î
îÐ7¢#? †ˆ	r"£?¯Qü…ÝÎ? †ˆ	r"£?"Åœ?‡fa—q^ô?Ž¸Û˜ê?‡fa—q^ò4FGL J1101.4+4108¿×"ð¦•pm@O¹É>¢ÒþÀ:{V'Ý¶À<~CyÒSõ@ ·~"Z•x?ú#¶¾mŽ?ÂÅ Æt+?ÁȚx'·"@´ªFJ@‡¶HüÉ¿ð?ïÿþˆ0»Š¿Õ'îdw"÷¿Öh…ºêw-¿áÇq^-O¿ÌɄƒ\ì?AGNbll3FGL J1101.5+4106RX J1101.3+4108?ïû£æÞP?V?E˜WùZ?Apg˜†¿)?V?E˜WùY?ï÷qÃd|b?cáf'2Ö?Qy7>Ý?cáf'2á?ïڊÿ
Ž?s ,Ð{½©?rº€}z¹§?s ,Ð{½£?ï{ÎóÅB?}`PbÆˀ?†<‡WÎ?}`PbÆˀ4FGL J1101.5+3904¿èWñWŒr@P
j½ãû½À:ÊbhÀ;ÛHHn-Û@å	Yšü@·Káâ8?½š)¡äì©¿£âX¥2©ö?ä¤d~.Ú@¹ññIƒØ?ïþ;â¿ë-i$†È¿çWöÌz—v¿åé<oŽ¿ïþ%–c.¿âïÃÙßAGNbcuCRATES J110130+390434?ïØ$Ä×?ƒ~Ãd믓?síôþ"¨?ƒ~Ãd믒?ïºãð@?—ó]5̔&?G8Ãüp/?—ó]5̔&?î£sªŽýI?ØŸ­3‰Ò?¥ÈÅW+m?ØŸ­3‰Ñ?ï}›†å?GNR6ô™?œ°]#q?GNR6ô™4FGL J1102.0-6054?áYz)cK¿éæúàÜNJÀ7äè¼í[¹À:!_Ìqç@ñèÒ@Èÿ΁Ù?¶Hê¿üÚ²?Ñ XšËÈÁ@)Á¡ŸØ?ø_Y	¸&?écáPè¿Å§¼Ýk€'¿æ|fÃÊÆ¿ê"eҐ[¿êZ³R¨D¿ÕcŠAGNbcu3FGL J1101.9-60532MASS J11015838-6056516?q]"àgÍô?­c,\¡?ïÝDØ?0d?­c,\¡?sáÐ_ò?~gì4}Á?ïÙÇè<_@?~gì4}Á?¡ë¾.6¹o?–àÃUº?îáD"i?–àÃUº?Î4Ú º´?O"ÖGQ?ïÿAŽY.û?O"ÖGQ4FGL J1102.1+2249¿ïø»ºˆlÓ@P;$_ZÙjÀ:Ö0ã͚RÀ<y,;È-+@øãýëÓ£@
…É=?Ñ:~¯"®?Ïg	y{l?ýæª|¦D@B9_E0¿•CÐå5Nk¿åg©\…<¿ç›Ò>%Õ}¿ï=ò@¿ïՀ/eHY¿Ó0æ"ÀAGNfsrqCLASS J1102+2241?ïïêa‰I8?eóÖlƒŽR?`žv¶Çž?eóÖlƒŽV?î\.µÜx6?¶¹½ôÒê!?ª=¢8|®?¶¹½ôÒê!?쩹0Ï¡y?¥è
?º²6y'ôF?¥è
?맚ê{µ¸?­¤Æþ@·Ó?Áa"V)?­¤Æþ@·Ó4FGL J1102.6+5251¿îâËQý@L¦&€IRÀ:҈
%ðÀ<ʵ1¥"@V7éPf@¹eç»?˜ùJ"2ª?Ë*Pv%ã?úI·¿Ža@xh??ߺé
55¿âÿ^šj¿ê˜±¨ó¿æ>mhc¿ïÿØȃ'ð¿éd}Ãz=´AGNfsrq3FGL J1103.3+5239GB6 J1102+5249?ïûåC¡?Hu"­¡-8?Aøk¢ñ¢?Hu"­¡-+?ïüNVÅÿ¼?O©£LŽ?=Iе?O©£LŽ?ï¿
†'r?'¤z‡?B?Ÿ(O;â?'¤z‡?B?ïù~©XP—?:Eo½.Ö?JZž½¦@?:Eo½.¾4FGL J1102.8-0148?Û~4X…ð@I~þ£ßm¹À;¼pñÚ£OÀ<ÏQÕQ×@#E@tI	?÷c¬bäÒ?×(§¾öJu?Ì<ì™.:?õâíÖ1Ð]@J}ғ¶¿ïÿ^à54j¿ï'7*8¸®?ïøÞ6A?ÌõýR.Ì¿Ðó~}ÖÅ¿ã8ì£^iAGNbcuRX J1102.8-0148?ïýè&:ñL?(F"Ì"ú?0¾Î(u¨?(F"Ì"å?ïü½Õ3?QÃÍ×H³ž?:YVgëv?QÃÍ×H³§?ïÛëe˜£Ø?qh¶'á£y?r
M3®?qh¶'á£s?ïõäàY«?H'èøòo?T7þ?L§b?H'èøò4FGL J1102.9-5628?ètÐ*Ő«@
J¡¼}Ê0À:p.Ï÷#¸À<¨(÷@ »a•qA@:ëÄØí?Ç8§?¸Ÿ.ê#?íè*Át©ö?ÿ?®3Yž­?ïÿ!Í°"¿ìTç4¿³[H¿Ñ*™¿á‹	³Ýè~¿á%&_楿æÔù è­ÔAGNbcuAT20G J110315-562635?ïõ¯™º©?]Ò,-~o?T ÌŠ­åc?]Ò,-~h?ïÀ"'oø?¡¢1ÑŸÁ?ÿ=¶Èß?¡¢1ÑŸÁ?ïµë¶åmÇ?ƒnÕÕw?'…F¤ŽQ?ƒnÕÕv?ïA·\/M?"ÍNž"ƒ=?ŸWÉz-?"ÍNž"ƒ?4FGL J1102.9+3014¿ÝõÓB¾B@P"
ú/§À:¢.›
³À<"îNý"@YÚ;JXê@!ï#8ê,?Äܸ¨'¦ã?ÀÖYh|?óQ+¡nz1@o%ý•—¿ÑW6]48—¿ê€O ý7¿é$¦©L•¿ìYƒßž
¿ï̚!ÿ¯"?âÉËûìu	AGNfsrqB2 1100+30B?梁%ÆZ%?Š@)Êêd?†'vŽiv¦?Š@)Êêc?îóÞêƒ!A?²ßÝåª>? ÂWÍëç?²ßÝåª>?ïy"æŽ?‡ƒP¤ÊfD?ß{£'®"?‡ƒP¤ÊfI?î¼
ºIÈt?˜¥Û"$Bg?¤?T[cx¶?˜¥Û"$Bf4FGL J1103.0+1157?îtÀ	k>@N6#=òªÀ8ø€'Š×_À<uƒ9ÛÄ@ÌwȹlÉ@aGãÄ`?©6æ'xÀ?¸ÿXÿåAÒ@
@-¹€@çÀI‡¿Ø9ã{î¿á¾«6z'¿æt~¢Gh¿æfOõá™
¿ë aÉÁ¿Ý™åóíAGNfsrq3FGL J1103.1+1155TXS 1100+122?ïü¢çg"?2þ†æ´ã^?:ï@ÄÆø%?2þ†æ´ã2?ïù!-0?[ç'dá³ê?I¿{·K>Ã?[ç'dá³ç?ï¦u]1Áš?"/zj«t?†b¨³™u?"/zj«q?ïÿ'ÊiˆÀ?‰Ò§7¬'?MeÐó?‰Ò§7©ä4FGL J1103.6-2329¿ïÀ¶Íæ>,@@‰ß¹8›RÀ9ï(ÝnۀÀ<![Ao6@ ø/']5?üNÞõÄ<Û?µ/Gì'Ü¿a*8'æÔ?«àÌVn@Y­í¹?íÕ»=®6_¿áâû{8†¿ãÌ?Ü¿Çïϛ´&
¿áÓìCÇ«?c…—ÓPAGNbll3FGL J1103.5-23291ES 1101-232?ïúÕA	]Y?;'©V¥¤|?Dªûڊšm?;'©V¥¤r?ïýP¶uA)?N×½Ô4£¼?5zLUö¹µ?N×½Ô4£¦?ï쎬H›?m•CW{,?cq€S·d³?m•CW{0?ïçÅí2aï?UÚìs?|?h:͞Ù?UÚìs?u4FGL J1103.9-5357¿œhüŸÌ‡Ç@š½†ìÀ83á
Ìq]À;Tª:э&@‰K+L‰ñ@-ÑyÚ·q?¢ß#í"¶?»p´yß@kK¯Ri@2("ž¿Ù"iʀA¿Õyœ^E¿ájè¬&d¿ám¬@eJÝ¿æœÜ¤Zé¿ê*ȀŒØ@AGNbll3FGL J1103.9-5357PKS 1101-536?ïú^/Î6â?Dpzc±À¦?F‡@Ç$~·?Dpzc±À¦?ïÁӀ>Ü÷?¥x€×Ô??à'".?¥x€×Ô?Æxé?‹&Ö·Âx"?ŠažW?‹&Ö·Âx?ïû…ØîŠ'?3#›¬'"?AèœE×eÂ?3#›¬'!4FGL J1104.0+2611¿»B®èa''@PØ¾r–öÀ;-C8dÀ<Ì]°µ?@ ԁ÷çX?ý?óÖ&ã?Ò+ݾâ~e?Á,á	š³u?ïUa%´Åo@Æ̝|þ¿ä9&A³¿ïæ,Ÿ›;Z?ì°Âtºg¿Ñ´îV,\¿ì^ܙÉjB?É/-5A*AGNbcuSDSS J110357.29+261119.1?ïö£JlxB?Q±¾ÒbI?R¹k'{†?Q±¾ÒbI?ïù9ý½Ç‡?o¤NÞÒý?K	áâ?o¤NÞÓ?Y}?ˆ"0?‰©¼ùá?ˆ"-?ïÁÙè/š?rYª`ž?èq3t?rYª`ž4FGL J1104.0+0020¿ïÈÛß4'@JiÝS¨À:ÕÀOæÈÀ<CHɝm@³k;p|@X¥}Ójv?Çg}'Hs¿'Âþ†r?Êd|ZÞs@Ga¶Scª¿ç¥ Jù"–¿æš¡¬bŸ¿à:â‰Ís¼¿îc!ãT¤?Æ8'}sHL¿ïÒìk΅4AGNbllNVSS J110356+002238?ïú]ƒ6ôæ?W&P"ìç?F‰ó$,dá?W&P"ìà?ïýÉȵc?J­¦0¢ä?1±ºWôè\?J­¦0¢Å?ï¿??7ë?‡C8¦=F??‡C8¦=F?ïúAŠ‰hì?@®à[¹ý?FùÕÚ\S?@®à[º
4FGL J1104.4+0730?èî4Tɪ9@Lùfb4¨~À9ÎÕxlù(À<RæP+'~@ת«dÈ,@ϋÃîú?±ˆŒÖ脎¿ŠÚ6ÓâÑØ?Ø.‹-Æè@ñÑØzU?J´·,Q—¢¿æT²^âc¿æWúȈšn¿àzó†tù§¿ã{Ö[åÚ¿è-ç>"
¹AGNbll3FGL J1104.3+0730MG1 J110424+0730?ïúí!T×ù?;ç"GÎ ?DKz¬ ã?;ç"GÎB?ïý°ð›R?JlR†¢Ùh?2x{%od¯?JlR†¢Ù†?ïê¦Ècp?umö((À÷?eY7œé']?umö((Àî?ïûôøÒ?.þ	í¾$>?@-À·×®?.þ	í¾$Õ4FGL J1104.4+3812¿ç%ÅÐS®Ÿ@PBIёXÀ5•v¡G
À:Óyq@'=ŒþU±?ûÄ£ÿYè?z}xf»?"×BÇzÓ[@º'®š²ž@Ô9ùËÞe¿Å¦²Ü¶¤Â¿Õ$è[Ÿ¹¿Ü‹Ù?Áa¿Ö¼/ʱ•¿ÞÙTšŒ¿ÓH__Œ«AGNBLL3FGL J1104.4+3812Mkn 421?ï\ÓOO@Þ?®"£v¬ÃD?"e–äG?®"£v¬ÃD?ï÷"i®ÿ?gõ~_D?PÙ-ö¢?gõ~_K?ëÝYjc!?¬›9Ôöð?ÀŠšVsïv?¬›9Ôöï?ïÿÙE3r>óT3RBé>ó]1fG|>óT3RD]4FGL J1104.9+5748¿è#Él¿'@K	pŸM8À;cpè hÀ<¿Pû›@Þs1s•@ÈPïܜ?ÃNwëC?NVq¬˜@	æ4á‰t¿í⯢št5?ïÚ==£#±¿í²•~æ¿Ò•!û'~¿ãÎCYñãÞ¿ïÿûÎBÓAGNbcu7C 1101+5808?ïþÂ"²{i?-±"'§×?#ÝÔØId§?-±"'¨4?ïýhƒf÷?M—׿eÉ?4»ç\ÈH"?M—׿eÑ?ïÞs§Q?"";µœÿ¿?œd=ы	?"";µœÿ¿?ïüRð½pH?4<èØ?=hz}Á_?4<èØ'4FGL J1105.8+3944?î¨Cï ô÷@P0O"}ŠÀ;/øìÀ<"Ž7£@N´¾c(@מà*w£?««u+%¿¶ï«^"[?ôÏ|ªuŠ@ƒ+ÍcJ¨?ïöaD=¿æ6M½øô¿è;$,/3¿ãÓø:8àò¿Á')™¿ç¥0 Y;ÛAGNbllGB6 J1105+3946?ïúð{'X7?@õ¾gÌ¢Â?D>ºŸÐ?@õ¾gÌ¢Ü?ïüÚ	»ü?PÄ[žâ$ñ?9ã/² !p?PÄ[žâ$à?ïÒNÎø~?̜7]H8?vØõƒÁÏ?̜7]H7?ïãsȾW˜?`^ܓÒí†?lŒ7A¨fö?`^ܓÒí"4FGL J1105.8-0731?ÚB6KÎ(@Gx ě¥ãÀ:ž'jöîßÀ<yÿ ^°@™½€Ô@ˆR]S?¿óâæ>¸Í?qbÿ»Ô°?³|{P®CJ?þ!/}F&Ö?ï¦rÅð9¹¿ä†ÿ=T<¿äûà^d¿Ù¦-¼%à¿áE}Ð:k¿èppçɨAGNbcuNVSS J110547-073235?ïêæÔ±(Ò?^@9À©d?e+N×,ý?^@9À©d?ïùGsèú'?b;ùý±Ú"?Jâ0\ÀH?b;ùý±Ú˜?ïëêÖ짞?kŎÀ#?d)Xb_?kŎÀ#?ï•Îì±?ryà-î:?Š»ŒDüSµ?ryà-î:4FGL J1106.0+2813¿ïÂ}<ç@P«hœ¡‹ÖÀ9TWuÇ,À<NÄ3¡<@ýñò¡Æ@®iŸÖÊ}?«ï°GÀç?²‰»ÀŠõ@¤m'ºZ@f,I	3Z?äQXí×ßP¿â	û+"é¿å±€`b–M¿åâ£cF÷5¿èۅ⭉¼¿æðÎ3Õ¢AGNfsrq3FGL J1105.9+2814MG2 J110606+2812?ïû‹Äí¥,?3D¼>1‡Ž?AÐìIkT9?3D¼>1‡x?ïüa÷Oc?Sš3nGd™??œðE"Ý?Sš3nGd?ïÆËÿI©Ç?z`Ÿ)¶h…?|š[+K?z`Ÿ)¶h‰?ïøK£—õ??qx7—ÖD?NÓ©q %Ê??qx7—ÖD4FGL J1106.2-1048¿¤á¤_Ã]@F$ÐgŒTÀ:÷!' ÿTÀ<U1Š¼‡@ôðVÝØ@Cœzª?Â\x¦Ú'¿–¬fzÞB–?Ò»-½þR×@¦`s^™¿ïÒ͖ h?êÜøɪÙ]¿âyJ]d¿ç#•Þùö¿Ô±JG
¿æk¿Á¡u†AGNbcuPMN J1106-1048?ïæ"<®Ÿ×?fŠÌ&ê&?ilÃQ`)¨?fŠÌ&ê%?ïüéÎö	?R2F—ù?8±ˆK÷·?R2F—?ï®È»-·?'®"ýâ?"MÑ4'>Ä?'®"ýÚ?ïÜùÿ_Ó?a]>Ò­—?qƒ~Ð?a]>Ò­œ4FGL J1106.5-3646¿âEmèó@5€"xÐÌ6À9ÉÌIN†À<D¨£!ؘ@IV
M·@ƒŽ)ùΎ?´}íì'Ô?³íóŽ¶@VÆž@
ï6ŽÝS?ïÿÐß´¿Þg=;tË.¿äø~+	Ë¿ÒÞc£",¿êJÔø³¿Ô¬Âû<ÍAGNbll3FGL J1106.4-3643PMN J1106-3647?ïù‰óú?DۅUjD{?IØ0¿"æ?DۅUjDy?ïöWmå?q©¥jÎx¼?SQ%þ5Ê¿?q©¥jÎx»?ïšÃý:?ˆo'póÌè?‰}Ͼqq?ˆo'póÌé?ïÇZ®w?d4®gUäÈ?|wÒ¨Äz—?d4®gUäÊ4FGL J1107.0-4449?‰˜8™e5@,hÆ÷ µîÀ9!—q¡-À;ã¬ÍSŠ@kêÈ5cd@lŒPû?²
	È««?Ñnîàå@¦ýòÆ@D€t¯_¿ÌN
$=H¿ã•è41_ô¿éÙ(?º*3¿ë"` SÈ¿ëÂbæ%z¿ïÿ£NNA¬AGNfsrq3FGL J1107.4-4447PKS 1104-445?îʪe=ƒñ?¢IËgG}?£UY¬'Àë?¢IËgG}?ïԞEgK?…µb†Týk?u°ÝLZz?…µb†Týj?ëÙÞ S?­}¨¦wBy?À›à…~³›?­}¨¦wBy?ïˆFŒ#?…Úumº
?÷.{'?…Úumº
4FGL J1107.6+0222¿Þ? ç:@KvX£/D'À9ÙÒø_øŽÀ<?x½€ÿo@¹Ggž@À¥ýU*Õ?´ÀÿÚÁ,¿Œ:Úzm?ØuzÖµ?ü]JÑ_ƒž?ï••9¹¿â$çî'C¿ä90m†X¿ÚÃ*¢8¿ÚA	8x¿ç0ãݵ}PAGNbll3FGL J1107.5+0223NVSS J110735+022225?ïӞo
kh?nTWÎL?v0ÈzÊL*?nTWÎL?ïèKÅíäs?{âº$)y‡?g´:‹Ç?{âº$)y‰?ïÈ,Ί4?zùͬ"Ÿ?{éþ˜ºå¾?zùͬ"¢?î³;õ½D¶?'	w$ðè©?¤Ì@¤+´®?'	w$ðè©4FGL J1107.7-3042?².ÀT3@;R¤ À:Õó‡K¹<À<u¿î¼@v™!N¯;@éœzõj?Âð¼@7¨Ž?e1Àz*©Ò?Ÿ˜<æÿí¥@»^ÃYÜj¿ÛMšÝ¼^@¿ÝǟÑÁÿ¿æ}‡ ¿ìTÃ;S"%?Μ­ 6Á³¿ïÿÉy[5±AGNfsrqPKS 1105-304?ïùƒáý¬m?O'–! Ç?Iðx	NGh?O'–! »?ïþ•)¾ —?E̯·æx‰?&­dö?E̯·æx?ï²÷È6÷¶?ƒvæÕ$s?ƒB
òB•?ƒvæÕ$w?ïýÐÑ;#8?(*5–ÝÃÙ?1yv&æEl?(*5–ÝÃÆ4FGL J1107.8+1501¿Ò_@ú@O‡EŒÒ
úÀ9À]''N#À<<Ò@ª;@+ÍcJ¨?ýÄÔ`?ù?¶šCžÌo–?µÀf#z@By<,9@0™)^"?ïÆ-vZÐ0¿àÿø¾m8"¿Ýw¥Þ¡`¿Õ7Í¡³ï[¿áp #‹öC¿åšíV°AGNbll3FGL J1107.8+1502RX J1107.7+1502?ï䂽7@š?cw}•Hp?k}BÈ¿gs?cw}•Hm?ïÂ;šg:œ?')Êô?~â2Ìb²'?')Êõ?ï¶òæJ÷?weöª›?'CFmz'X?weöª›?ìÝ÷2©\®?œ2Ø/ç°?¹Fjµ"?œ2Ø/ç°4FGL J1108.7-1844?·êçOû@BçÁß3ÞÀ:Ò
(ÝnÛÀ<kDTæ³@¾òÖ§l?ÿž\\!i?ÎÏÅåýËG?ÂU½ ÝE@?ò®²Jj‡]@Z©è"8?Ò ~:Bœ¿ãOäÿÉy[¿â˜¶DË¿ç¡â"o¿Áô×ÃJíå¿éø@~AGNbcuNVSS J110845-184505?ïíåXg ?`Ò]ø?b€§˜_?`Ò]ò?ïýn çù?N‹‰w×o?4ŽÿÀ.–?N‹‰w×k?ïÆ$gbž?|֋9µó?|íÌwαY?|֋9µë?ïɬÃWÜþ?iêužð=?{)žTv?iêužðE4FGL J1109.3+2411?äø±Æà(@P¶'Ìö¾8À:?9ÉOiËÀ<g¨"1 Œ@ 
¸÷'Øã?ýwM©Öþ?¼çýÀ4¸ï?¥uø)Çύ?닫à.@[¨ý?ëÄ'¬í3u¿Û懞olI¿àÔN¡MÿÖח`Ú5k¿áüÄʟ̿̂ XÐ{®AGNbll3FGL J1109.4+24111ES 1106+244?ïõ5 2>?I/b[r?U•¿›ƒò8?I/b[Œ?ïúy	‹?^	öÿçØ?GãúÙќ?^	öÿçÕ?ïì/ZT×?kû¿%Æ?cèÐ¥«)R?kû¿%¼?ïËâ6‹•?t 
Ûf™?‹Ír]s?t 
Ûfš4FGL J1109.6+3735¿ÅVIZ…sM@PŒ°á´»^À:¶'néšÀ<…ý	«zm@ óÿ'¥?ù,Ø:¿¯?ÐKs›Ù?ÈTµyt
>?ø7ó÷´$@	àŸµg€m¿â¢X_g™—¿ì곝PÞ?¿ÑO7
XH–¿ÓØLÝ©=ü¿ßŒDý
,T¿àcŠØûAGNbll3FGL J1109.6+3734NVSS J110938+373609?ïþ&Üâ?%³>¦'«±?&/͒1̲?%³>¦'«ž?ïü׿0$?QìPë`
n?9B~ßm?QìPë`
"?ïëÇ,¼Ï?mFN}wÉ?dç8ÓC1U?mFN}wÎ?ïøúp œ>?:°KOE?L=}®?:°KO4FGL J1109.7-4814¿ïÓ¿Q³j@&êþæûLÀ:³þËLš
À<ËRyI˜@øS*I¦@|š»É.?Êh'äÄeJ?Á	pT§?óøÜP'`@í}ÃOJ–¿çÕ\¾Fø¿àPVXÍ÷¿ëbâ¸Ç\K¿Ý©àc­y¿åzэ%íпïÿÊPʇAGNbcu3FGL J1109.4-4815PMN J1109-4815?ïøÃÆø^?TÀ­§Ã?Lðä‡'3?TÀ­§Ñ?ïûʍ"í?cŒîXáÓí?@ÕɲIÎ?cŒîXáÓò?ïDրv*?ˆ­~tkÝ]?Œ.Ê_âu£?ˆ­~tkÝZ?ïï	ù0ý?Qÿrãe¢U?`öìÏ™?Qÿrãe¢E4FGL J1110.2+7135¿½¹^)ǯ3@E°U2a|À:m«|ðìÀ<­ú4ää@ ÛN?üºØÿ
6»?ºŸJžê	?ÀÄø(e¥@Ÿãåî@æÏ¥DG®¿îfºI<‰ô?ïœàÁ q:¿È¶ÅúJ´Y¿ÚI›)'Ÿ¿ç*J+Ú¿¿=ç—({AGNbll3FGL J1110.0+7134RX J1110.5+7133?ï𺾶Še?bá<»ëg?^Š''ë3×?bá<»ëh?ïñVÿzm¶?s&v^O??]R$"œ?s&v^O@?ï¹ætªpr?"Ëӑ~²?†bÕcãv?"Ëӑ~±?îŜ‹^?Žµm™KÅ)?£¦7JÊ?Žµm™KÅ)4FGL J1110.5-1836¿Òp B¨Î2@CÜ­¡À9ñb‹"À<0îP«?@ .l6˙?üo"èbT‰?À7¡?Æ!w±<y@ûB±Á¯@š#SAE›?êéTWp)^?äšs´,Â׿à´uBwHâ¿Ú{Ϥmˆ¿ÞìTQì¿çGpÂ_ágAGNbll3FGL J1110.4-1835CRATES J111027.78-183552.6?ïåÆ«<æ´?eMKbè>?j9TÃKì?eMKbè=þ?ïø}`æ?dy#áª_?Næ|gæù?dy#áªY?ïpÄÝ`C	?÷ãë+O?'çdS÷ž÷?÷ãë+M?ï¬+l2Qè?p&	ó¦M?"õ$ók…è?p&	ó¦N4FGL J1111.0+3542¿êÌc#Sòx@PÁ)^ž	À;Qχ'0À<ݐ8ÇǪ@ BÞ£Žåá?õ?\l¡?Ý8LA÷ò?ïñð"<jê@ϵdÑ:ñ@Æ¡Íš¨?ï¦Vv.Z†¿í³Ç™kv¿Ê¨# 8Ü¿ÀœaJÙ«¿èÁUj• ¿ìcõrÞCîAGNbllFBQS J111056.8+353907?ïx'lÆ)ý?"¹ë¢Õ?ûg:ÀZ?"¹ë¢Õ?ïbNj§0?°ÒR¨ðè?"¶?«Ú?°ÒR¨ðè?îvŸc,ƒ­?œC-¤ÈœÃ?¨–	Í7ÅL?œC-¤ÈœÄ?é¾vö¹N?µ'¸Eœ%–?É$%È?µ'¸Eœ%–4FGL J1111.4-4624¿íóÁ»ÁÖ@*œÜD9À: Ô`?ùÀ<-±2ã@gò'"ï@Zp?Ñ_H$†òù?ѵ"2E?ýü+_)[C?þû0ˆ!¸?ã¶i´Ï€¿çàæ_E	õ¿é–'q¬ë†¿â¡¬­O"¿îÁ
F9 5¿ï6¹ÐpÆ<AGNbcuWISE J111127.39-462504.0?é8P¸Óv"?Åÿ*Á,ŸÁ?˽²'u?Åÿ*Á,ŸÁ?èGô­?Í(ø°"'Ö?Îãè-KÇÆ?Í(ø°"'×?èN9ãšUë?´Ž–N§z?ÎÇq–¨S?´Ž–N§z?鄝/¼°?®éýC`ç?Éí‹A…=?®éýC`ç4FGL J1111.5+3455¿Î
Jµ¤G‡@PÒ¼j~ùÛÀ;pZÇ̲ÌÀ<¡`†R"ø@"Ç~Õs•?ûr
—~?ÉüšoØ¿[÷7	B?{yïÃê@€(R¯zW?ÖIë;LÝ(¿ïþåþ÷í7?ïÿüÚ±'Þ¿Öøè^£¤_¿Ýî2BrkW¿å»l°Ú(AGNbllRX J1111.5+3452?ïþ"ƒl?%÷]º],'?.íß7É-´?%÷]º],?ïýO"¿øæ?L®VÕ¯¨?5ƒb8Ëq?L®VÕ¯¯?ïø8IŒ±?KûzâD2?OہÍ>R?KûzâD|?ïèè…"€†?Z˜(Tkp<?gzÝy?Z˜(Tkp94FGL J1111.8+4858?ì`~hÿ:@Nu>ÄaÀ;׳¾
ëÀ=µš &@!Yy²s…3?ð4Âkñ?çÒÕZ::?ßê^bá̎?ôéËº~@ò00õ@^?ïø÷Bl64¿â~p·'©¿ïÃC·õf?îVų-¿Óm'©èò¿æjmAKúªAGNbcuSDSS J111158.89+485701.4?ïþ~±dj?,R£"?(ï9¹W?,R£"^?ïý«4ý$#?Lj6çÿ•?2¦XÞî¯?Lj6çÿ»?ï±³T¾SX?""k»Û?ƒ"*Ðk)Ý?""k»Ú?ïÿ[ß`:'?Ÿ´;(š?"ø»$-?Ÿ´;(d4FGL J1112.4+1751¿ë‡Vž®L@PX£/D'*À;%ö4À< ÷ÞÉN"@››``"@ÄɅðoi?¼Áw녿´ÓœIÍ('?ûdÏÃ!R`?þS…~»÷¿¢-ï7Я¿æÉ	><Þ¿åü8§ç:¿Üg&Ɖ½¿í	}£~?çœÂñAGNbll3FGL J1112.6+17491RXS J111224.2+175131?ï<[)?†Ã÷²'¥=?°é:øõ–?†Ã÷²'¥=?ï"k»ùz?ª…gƒü?Žå>Ñ¡Ï?ª…gƒü?ïpÌC~ÕN?‹Ÿ
c?'æw%VO?‹Ÿ
c?îØ E>?'Rz?¢Ö?¢ö+¬#?'Rz?¢Ö4FGL J1112.5+3448¿§Í*viA@PâBؤUÀ9L p¸ÏÀÀ<!@ÏÓèJ@Œiƒý%/@ô¡ã6ï?ªÉSE¢Kš?›Wߺæ@$ñÃ&ZÞ@eMÌg¿Ó¼¦Ä¥`ø¿àÉqޔ a¿çˆ	¹½%¿éœ
V›¿éMnÂs-¿ïçâ!´†AGNfsrq3FGL J1112.4+3449TXS 1109+350?ïõ\j{~ß?Qðä۔ à?UG+	C'?Qðä۔ ä?ïù»ˆ'Ò¼?Zþ©Ì74H?Iß`µÂ?Zþ©Ì74A?nrm-?"õ¥xì}c?ŠRdcd´ï?"õ¥xì}]?ïø!v3%??¤z×UÐ*?OÃz'3i??¤z×UÐN4FGL J1113.6-1920¿ïû¶ã›@Bë ¾Q	À;›r·®À<"‰†üÞã@|€3>q?ú''Y4?æõ2ôD
?ØbëóÁ{?õú%zãËí@VɩתK¿¯¯EAA'›¿ìä>ÙY£
¿»ÔyŒ]ò¿àMt'yè¿ïúïàM28¿ïÿÿ>¹úAGNbcuNVSS J111348-192252?ïþ{Œ¢P?3˜Ý1­ÔI?(G5Úÿ¹}?3˜Ý1­Ôu?ïý±£çõ½?LŸBè?2ràÀR@?LŸBà?îíL']yJ?•öSA§?¡+=Š(kT?•öSAª?ïú¨+ˆ_%?8x¤ëGŠ&?E_Qރgö?8x¤ëGŠr4FGL J1113.8+1528¿ìS+Š~@P!¼ÓZ…ˆÀ:õ'R}À<˜s%³@k֒ÉEÚ@Ì_¿ƒ8.?ÀÞº z^k¿¦âSÁÊ?眐úŽ¦÷?ùræ‰âA~?ï›îs¿ìCÑ¡ð§¿ßJ¨/^']¿ßæèArf$¿äw4cn¿ß-¿ÖÅAGNbll2MASS J11135586+1528058?ïèF¿k…(?aUÕ»dÞ?g¹@"z×Ü?aUÕ»dÞ!?ïÏnžòý*?vW@¬à?xH°†k
?vW@¬à?ï¦îø–""?ƒƒø½šj?†DAÚ^ßH?ƒƒø½šj?îwŠ°
Ö?–3cAµM?¨‡Tÿ/R?–3cAµM4FGL J1113.9+5523¿ë.=¸‹Š@LX[žŒG¡À:Ÿð+oðÀ<ÎeÅV¶Æ@ïÑÃ=­@]'Z
7'?À)§Ù£Iò?¸HÈEÔv?ù@ùª{i-@¨âºtÛt¿çuB!b¦?°'×5[†¿æeçñr¿Ô:Ð`€r¿ãž"Ք¿ï÷އŠMAGNbllSDSS J111356.29+552255.6?ïû ސ??åb¹N¶\?A‹~…½'??åb¹N¶g?ïû`
)Ý?W õ$'Lx?Bç×XŠ˜?W õ$'Ly?ïèkõÊ?p*+Ò¤ËÕ?gâ"
ê6?p*+Ò¤ËÔ?ïÐá/"£?e	®©‰ëž?wh|¶.¡?e	®©‰ëœ4FGL J1114.5-0819¿àÍAý±¬Ž@G¾Cªy»®À9ԙœØXÀ<+£<±@<Áz^?ü@CßâSG?ºÖ<!ÄJó?ÂL;ÂÎÇ#@­·®W–À@@à$ÃXÛ?拝'uß¿çƧÿ¸ÝW¿ê)!¯íï¿ìäÐ.Ë¿ï¢£Y6¿ë¾hêAGNfsrqPKS B1112-080?ïå‹ø¿
Ž?lµ"U3z?jt@õr?lµ"U3u?ïßR<RHð?'Û'[¯L?pVáÖۇº?'Û'[¯L?½´ã?"]ž·M®?Œy'Ç?"]ž·M°?ïñíÇ
í?ˆÓ‰,ÌBç?œÂG¢[?ˆÓ‰,ÌBç4FGL J1114.7-0248¿ìG'#™ùw@J¨~8ëÀ:EÏÞ²À<)œ1úN@&¹¶ðl@òÊ!÷¡?ÃúûHáb?¶y"˜€•?ð™šäó?ÿàTyá?ÖBˆCa¿êÉԕ*™¿è±5Ý\'ü¿çӄ¼¿ïý¸'gù¹?ÊöÖ-ɒAGNfsrqPMN J1114-0248?ï°øå%?‹…9ÏWñ??ƒÁú¸¶ú?‹…9ÏWñ>?î†/'òÎí?´Îˆ'?§àÓ<?´Îˆ'?î-þ?–l½QÑ~?¡µ- )?–l½QÑ~?írÍè!¥?¤g'¢?´i¾óòÌ?¤g'¢4FGL J1115.2-0703?ÑÚ&¤td@HQ^	À:XaÀå8À<Lk"ÌÐÿ@ò;"™¦@@"Eð?ºÒ6™A?¥&¨$:¶¤?çވì£+ê@ÆâCV–æ¿æƽêî¿Þ.dß¾—¿åÎÆ×ÀEÖ¿à-î$nt¿çéŸ"w¿ÙÀq_=ÓAGNbcu3FGL J1115.0-0701NVSS J111511-070238?ïö^Ø´CÞ?P‡=1??SBN—xF?P‡=1B?ïý(¹q5'?Iô_U•¥"?6º4vSx­?Iô_U•¥¨?ïê·¾YZÿ?lôÛc]T?eHA¦¥C?lôÛc]c?ïé)"ù¿?T…áÊÈ"?fÖ{å?¶?T…áÊÈ4FGL J1116.6+2915?ì'<Ê÷!#@QB­­ê‰À<Kl»êý9À= ¤&ó@#¨©Úî¤?鐗ÈAî?ép›Þî7?ê~e`¬é@"ÄæN~@üiÙ¿ïÿùSt?ê‹ùæ/t¿ØÞ|øy#?ï¡æڕl?Ì«IYæ%c¿Ð2":¯ÔDAGNrdgB2 1113+29?ï›ð5GE?)Ê?‰ò®.½€?)Ê?ïøö| ÝÜ?q(¤P†Ò?L&|ˆ.?q(¤P†Ò?ïB3¶¨§{?'Ù¯æ"†?—¹‰*ëÈ?'Ù¯æ"†?ïõ‰¢@žI?U^Å
ò¯Ü?Tì»~Ãkë?U^Å
ò¯á4FGL J1117.0+2013?êk€«|Û$@P×j~ùÛ#À8úùåܞÀ;ï*¯ÖòÀ@9 Va¶~?ÿH"¹7Ē?¤œ|^0ž?Q~'œRç?±"÷¦À½@±pÿÇuö?ϗ#k"ù¿ããpè gê¿áE†òÍè¿Õ掿ËÝd¿äο€³ï†¿Ð.feÍxAGNbll3FGL J1117.0+2014RBS 0958?ïÿ8™Ÿæ?ùŠQv4?ØìÌ0K?ùŠQv3)?ïý¥ð!A"?Ksw¾É-o?2Ð~õöó¤?Ksw¾É-'?ïó¯Ð¡ä"?eÿÏZ£[?X ^¼6د?eÿÏZ£f?ïÿ§i'>÷‹ªßÙ֖>þ¬K|·"F>÷‹ªßÙÝ4FGL J1117.2+0008?¾ÊÌȃpò@Kcí¿‹›ªÀ:÷k:
½ÉÀ<Š|@Ã?@ ¤É'PÑÕ?üº¡6F
+?Ë­=¾§p?®|>>ÿð?â®q,"@µ+‹¿îÏõ@‰]?ïév†oj¿Í$¨ҿDžþ²"&›¿éÃl2š‡?֖K›ßÄ÷AGNbllRX J1117.2+0006?ïýXÉpLG?2*"°Ï?59´}Èl?2*"°Ï"?ïüffUÇ´?U&·îå?<ÌÍQÂbÈ?U&·îÙ?ï"×:N]?‹ë"ü?äh?‹
?±lhd?‹ë"ü?äi?ïêä{ö¶]?XŒ™å(?e"	I£$?XŒ™å 4FGL J1117.2-5337?ïÐãòM™Ú@ÐO±;`À9ÜRX'hMÀ<HjÒܱ@¤ëg†ù?û1GÏ¢j?¼+‹tõ¡?Ì´ªV«2s@…Ìe÷@ºe+'÷?î©¡ÙY"¿ä
~q ¿ÓØe1]¿Óޖ"ì"¿á̈¿V"¿ïÿ'âH	.AGNbcu3FGL J1117.2-5338MGPS J111715-533816?ë2&›Ç²'?ÁTøRÁ?Ã7eá5»?ÁTøRÁ?äPûB 
?ÕR¡fÙÉ0?×^	{¿éë?ÕR¡fÙÉ0?砍aà?³zÁCÂÒÙ?оåÁ=à@?³zÁCÂÒÙ?ç7q Gêí?¯оÍá?ё¿p*&?¯оÍá4FGL J1117.6+2550¿êa·ZQÀ@Q@9Õä¤À:tu;ÄÀ<šk‹iU.@úGtª@Í]…U?º]âžÆ)E?Žê¾¶oÏW?Ôf˜:@YYBfê?î†òBR5¿âÂÖ>e–]¿ãæÅÒÈq¿ãµDD¿æہÁ
̸¿Ù¥W½×žAGNbll3FGL J1117.3+2546RX J1117.6+2548?ïÔԏ'&?nÑèúu
¢?u•÷8llÅ?nÑèúu
¯?ïúl)ªS—?e &§'>¶?FOYV±©&?e &§'>®?ïÖ~Û½>Ÿ?y]A³®El?tÀ'!`¯A?y]A³®Er?ï¬áƒÇvö?q$ßT;š?"ÇŸ"B¤?q$ßT;™4FGL J1117.6+0217?æ8ôyr"@LBŒi/nƒÀ:Èût€À<])4¬¯÷@S¹¿~Û}@ ¶fXúm?Ä\HUYMÏ?B»ÆÇúl?¡Þ.ÁUí•@gÕR­Kþ?ïtŠˆ×¿â'~e'¿é´*¿qD'¿ÕØO¢T©%¿ë8ë¹4¿ïñÂàÍ=AGNbcu3FGL J1117.7+0217PMN J1117+0216?ïïõ­í÷?]ú
ŸAa?`
Ræž?]ú
ŸAi?ïüñ:Vß?O$ìÒëA?8v-KZ?O$ìÒëF?ïÛW½Ÿ¾?w×kÎ_¿?rT}!0!Ý?w×kÎ_º?ïæüué?Uä¼)f·ˆ?iŠàéI?Uä¼)f·"4FGL J1117.7-3650?ïì'n¦¿P@6Y~™cõÀ;òø°€fÀ<"ö(æ©@Ҏqó7p?üãx«ˆ¤?Ôo›-îOÔ?Ó.¹PïÝ?ûUȤI @}´üvˆ?ïÌʳíض¿é0ç"øoé¿¢è&šs‰:¿Ý[5ZÕ¹…¿î¹Þ]˜âe?ÕX@2õö'AGNbcuNVSS J111758-364918?ïñ©-*Ɋ?a%¹LŽa?\­¥ªlïV?a%¹LŽ_?ïËԁ"y-?'·:xùU¬?z¿5ÃhÕ?'·:xùU¬?î;®.¦¬€?œ¡ðˆý?¬E•7ö?œ¡ðˆý?îÜ9ÅÁЂ?¤©aH£?¢<c£â÷×?¤©aH£4FGL J1118.0+5356¿¢ºýÈÂgÃ@M¬ÿ§ëlÀ9†S³Ü;À<"û¥'l@"J"ú?ü‰ÔÊÈÏ?­Ÿ¶¿Zð?²?Mȵ»ä@_íQx™@‡k'–Fÿ?ïÐnýäœÍ¿"
ñ)¥…¿àWŠáÅ¿×h^ùŠšù¿â.î%)¿Ú½_œr¼áAGNbll3FGL J1117.9+5355NVSS J111757+535553?ïèßà·aì?c¢Û@Iok?g Hž>?c¢Û@Ioi?ïӌ_Qx?‹5¯÷Lo?v9±PWC£?‹5¯÷Lp?ïr
'Å-L?¸áv&Í?'¾­§ZVu?¸áv&É?íµ°¥{\Ö?"r&õ°Œ™?²RzÔ%H?"r&õ°Œ™4FGL J1118.2-4634¿åÏOë *@*«nø_»À:ZëÞàÌÀ<3ˆ˜`´@¬Q'M›@TªFJ?Ñ4òÛª5H?Ú$&»U¬@1[µˆ@(t,vÖ?ïövêB(™¿k»Ý2Âí¿çòCŸ'Æ¿æcçeÕFï¿ç]13~²Ž¿Æg³'ùÄýAGNfsrq3FGL J1117.7-4632PKS 1116-46?ïï=Œ1?¡™Öö'?œbNyÝQ?¡™Öö'?ïŽÜmµ~?§wçqü?ŒÈ䒠3?§wçqü?éñ*£ÿ&,?­R`Õöê'?È;UpgQ?­R`Õöê&?î‹Ôáš?•…Wö¯£ñ?§B±æ_ß?•…Wö¯£ð4FGL J1118.2-0415?ﮃ¼Ø'@I²@(äüÀ9¶<ËbjÀ<z¹ÚÁ@ †ôü@Ù@ÍG¤ç?·ë'ˆþì°?¶¤?	ˆ?ù+õQP@|@BeU¿Ú rÑ®³Ý¿ãá01 3¿è—è¿qšw¿çœ'aï‰:¿ìÓfQÒ[¿ï"Í®oêAGNagn3FGL J1118.2-0411PMN J1118-0413?ïýӜÁ"?/QFŸÐ…Õ?1c÷›_?/QFŸÐ†^?ïý&δJú?Ixl½ŒÆ}?6Ɋ]¨5 ?Ixl½ŒÆ?ïÙFŽÀ@w?súÌ5ׅá?s\¸ŸßÄb?súÌ5ׅì?ïÿ\>dÕ?	ÎîñÑ=?x=se4ž?	ÎîñÑ;u4FGL J1118.6-1235?ï%7‹Sõ%@F*䎊qÞÀ9öñûÀ<;Æ*\}@ÛÓöeM@Hæùž¼ï?¼±;aU"?Âj‡ÃŸÒ@	Ĩa³@8÷¯#™?ïÿÿÊPË¿çîG;'ô;¿ê|Vþ–¶¿èӃÕâö¿ãÏò@Ϩõ¿ïþ,UÉ`1AGNfsrqPKS 1115-12?ïüc U?BCGb>¤«??DâÿÝ[¥?BCGb>¤˜?ïÐæ}?™ÞÂ(|?wŒþvÁ{­?™ÞÂ(|€?ïi_TÖ¡E?‹ùu%Pš?'Ôe+×f?‹ùu%P"?îñ¬ £^Û?C¸#Ç-? å5õÊi?C¸#Ç-4FGL J1119.0+1235¿í'Ùž›Ü@Oø·`,'À9íÝ{p¹¦À<Þzt:@%ÿµØ>›@=ðüVþ?½M6êwØ?Í^#vҚA@3xî(g'@
~w)W<¿ÂäÏw÷ÞH¿Ý8e˜º¿çÊ3ß3W¿ê¿cW¾-¿ïþÖj€˜?î§<_VÒ AGNfsrqOM 127?ïÎFRצ?}½ê4¿y?xÜÖú,˜?}½ê4¿y?ï÷׉µª²?bXo#êºñ?PP씪š?bXo#êºò?ìeƒ¼š^¦?¥u>`™u²?¼Óâ-
Ð?¥u>`™u²?ïӘçÈÁF?jœ]G­j?v3ŒŸ\Ý?jœ]G­o4FGL J1119.6-3047¿àT‹˜'@<ÈæŽ>óÀ;c…LXžÀ<´)3Õðb@"/sš×\?ü8ÇÃ?ǂ´eLàÙ¿˜Du?Ò¼Ú;uL@'®¨—›¿ÕÀæå|Æû?ïÜE É
пë{;	ÁJ¿µ59È£T¿×ö‰Ÿ%Ÿ¢?țt$¿ýÜAGNbll3FGL J1119.7-30461RXS J111941.0-304652?ïû>í°s¬?? KÁ¥d^?CI>1T+?? KÁ¥d_?ïþ:9G:?D©Ž\v¡?,\n+Œdk?D©Ž\vŽ?ïážÉŽþ?l'"‰Îc¿?na6åq¼?l'"‰ÎcŸ?ïô›·"-?HpN…Îß?Vȑ»¥â®?HpN…Îç4FGL J1120.6+0713?ï€/ú¾‡@NV0U2a|À9ä(rÀ<P)Ôà@˜à¯à«?üÉçÅv—6?¾Fa8T/W?ٟúdŠn@XÿI Û@ˆj$aY¿éŠÐ=š•B?Ð6¢~oœ›¿×>adžæ
¿â¸J"xÈi¿ïÅ<¡?ßjÊÄ^êAGNbcu3FGL J1120.6+07131RXS J112041.6+071335?‹&º¢í?Ìét³?etJ?Ìét´?¬zÉ9ûö?¾Ü6Wqõ,?î8Sl`??¾Ü6Wqõ,?›©SýÖ¢å?"!"±ìç?ï"µ`Jê?"!"±ìâ?¶gôù·:|?§GtGÍ)?í3`É°?§GtGÍ*4FGL J1120.8+4212¿ÌF I›C@PŠk΅3±À8ÁA÷TðÀ;¦. |w@ ¾ØÈ.?ùÀ¿xPt?¤wÉ¡Zii?§`®>@eŽšbv@tmoïüþ¿ç'E'ƒ¿Ï²¼•ÇýۿՄ½A¿h¿ÕKí^'²u¿ÉHY`™¿Ñ+¼üKAGNbll3FGL J1120.8+4212RBS 0970?ïÒ9E"!'?sÚ¾¸â•?vã]=ï>Ö?sÚ¾¸â•?ï¼p7Ǎ?šjðÔQ'?€ãزy?šjðÔQ'?î:ƒ:ï? þJhH?®^ÌQ? þJhH?íF±Ë"Üð?¡œßֈš?µÊq£Ù'?¡œßֈš4FGL J1121.3-0011¿ïÑÀf/Š®@K"Q´þÀ;ËñºzÀ<œdÐd1@ Hƒ}Îaø?ÿ"à°«.?Êϝ÷øµ?ŽÚÜs͛î?Å£øSY@ҍٜéÛ¿ïÛO¡ÓÏË?ïý…Ò<xV¿ÛeD¨P—¿ä6"Ü¢¿ÃÛ-¸Ÿï¿è;¿(Ÿ[zAGNbcuMGC 0019706?ïü`B¢Á2?;´Ýß°?<ýêéögô?;´Ýßí?ïýÅâÑW?Hcï•ž\?1ÐéuCè?Hcï•žH?ïÑùÔu9n?wj>£h"?wÅcIT?wj>£h~?ïéþ˜=ˆñ?XêLÅò`–?fgÂw™?XêLÅò`¤4FGL J1121.4-0553¿æ%ÖÒÅ®Ÿ@I9PüqÖÀ8¥Q­DqÀ;Ï×ð}ñ@¡sÕB<@x"¡¸?£À–2±Ù?Á£~õ©dé@Sžã…v@ƒaòåæ¿ÍýV
㘿â°]ˍ1¬¿å*Ú~çÆ¿æÀ–]¤öÅ¿íƒ|V'³Ì¿ã$A"àAGNfsrq3FGL J1121.4-0554PKS 1118-05?ï¹K]x(?ªößMáïÆ?­:¨¡öC?ªößMáïÅ?ïîèNëÑ?q}^i9_?a±~.??q}^i9Z?ïW頔J·?'k…»]O†?•Ëív©/?'k…»]O†?ïÙËÃöb¸?`La-Þ¢s?sΣñ?`La-Þ¢w4FGL J1123.1-3233?êóÆ,ìX©@:¹Ñ¢£YÀ;–m•/À<žÉ¬†Ü(@Rž˜†ôü@óý]ŽP?ÅÁ¼"…ù?‹†ù?Èòüvރ®@‡A 3fµ?î=ï^òÿ'?ï§$f畦¿ì)õœÏ®ÿ?"×Bz+Æ¿ÜKóÞßsî¿ïÿõž}.)AGNbll1RXS J112318.0-323219?ïúÊ6j¬Õ?A†Eq¾¾Æ?D×&UL²`?A†Eq¾¾Ð?ïýù"ÃûÝ?Jöæik'³?03Yà!£?Jöæik'©?ïӊ'˜{Ó?ubfˆ¯'a?v:¾³Â¹?ubfˆ¯'k?ïí%º'2j?W(<AÖÎ?bÚEn͕@?W(<AÖÕ4FGL J1123.4-2529¿ëÌ$î—@@£Þzt:À:´É.4À<Q¤Æô@?ÿòˆJ¼½?Ë,Xãñ×s?Ó¢šÛ¸ù@j[¾l·¹@«_ð«y¿î´@ÿ¤n?ïý_;Ϲç¿âFr«G¿ã¢$'–H¿çêèÁŸòú¿ïÿß~€8 AGNfsrq3FGL J1123.3-2529NVSS J112325-252858?ï÷'$AÞÕ?Qt%7țã?Q±·|BR¡?Qt%7țß?ïûiÞãMô?^~¨¸5Ü?BX"rÈ,'?^~¨¸5ê?î'á1œ\â?˜»rŠ 4?¦áìæ:1á?˜»rŠ 6?d¶mÿ"?oúxÂ?€žÒd€F?oúxÂ4FGL J1123.5-6418¿Ã™F6Œ"À] Å®À9ªkµZÀ@À;)Ì¢Ûb@¥'—H±@EKc¬?Èaq	,¤y?¼ðò›éU?øyìU(Q@¡¨ä»+?ïÿP3:¿â¶CÞÒõ¿æä%®æ2¿ì	tÞNTw¿è(úà†h¿î–JŸ‹vAGNbcu3FGL J1123.2-6415AT20G J112319-641735?ïý5㧘x??k"(¼º?6PâÃ<B??k"(½
?ïýW2®?Zá‡Ñty1?75Foꍶ?Zá‡Ñty6?îÝÈ´nà?˜#Ïlèòr?¢#~ô¹ú?˜#Ïlèòp?ïÚš6'/?a
<Ò
XY?rø²ä¶è?a
<Ò
XU4FGL J1123.6+8028¿´~F
ӖÑ@AótÝÛÀ:Øý›²yÀ<ÍK
P¼@o*|«L?ÿ³vŸ™Û?ËO äüïT?Õê{´V^@>À·pD@ÖèÚt€¿î''¼¨'?ïùx&'JÈ¿å‹ZÜÅhT¿Ù'D:Ât¿î­¿jäz¿ïóHa˜¡LAGNbcuWN B1120.0+8046?ïc?σ-4?'†Iã??"˜šY¦?'†Iã??ïjN»e¯~?«(^ÂXšš?'¶("J"?«(^ÂXš›?ëô©kq?©¬v²-i?À-[›šR??©¬v²-i?ë'á´8݉?¯?>–g¬Ô?Ã`y/‰ß?¯?>–g¬Ô4FGL J1123.8+7230?ïoچzÇ£@EŠn~bÜnÀ;œ®¶aP}À=¡'Œ_@!¹üøä'Ì?øÃæÄŗN?Ê-˜),A?ɀ1©k@óH+è¼?õöA»6L¿ïÓèë"³¿ï¶R¢dCv?ïÿÂWþÅ¿×î]@L÷¿ßx`cíæ"¿È*ýD8êAGNbll3FGL J1123.6+7231RX J1123.8+7230?ïùïôOÉÖ?Mx»}¿?H@.ÀØ¡Ž?Mx»}¿s?ï»æ¬Á¤p? ¦8ª÷çŠ?Tϖãñ? ¦8ª÷çŠ?ïcè£ÏÞ?Ð¡ÁƒI?"'ëæ?Ð¡ÁƒE?î@¹BõàÜ?žYœÌctG?«ôkСòE?žYœÌctG4FGL J1124.0+2336¿Æp×s·'@Q~Æ"§À9ìú'è},À<-:ƒ‰ŒÜ@¹ö¾ëv@Bá¹Ãۍ?³ÌÕ±!öu?"Tµ ¥?Ô4ªžP8@ž{Fó.‹¿í'ó*ö?ÌÒE݄Õè¿ç$ŽŠqÞj¿ãi!Œ—¨¿ä
':ƒŽ¿çø— B•§AGNfsrq3FGL J1124.1+2337OM 235?ïֆ—HÔ?u<¨z«ü.?t¼õ4[•@?u<¨z«ü2?ïûÀñ²@æ?TÔçbœ ?@ü96üh¢?TÔçbœ–?ïT`3Ïøo?'*¿Äð7?•sù†ò ?'*¿Äð7?ïȋ;—•(?m/¼£Ð?{ºb45kÚ?m/¼£Î4FGL J1124.0+2045?ï
Óyªë@QEy¿ß~€À;Ù¦ÏãÀ<¢­\Äüõ@ iZA"ö?þ*ål[?ÍÆ^ˆ¦?´¦ùS"{?ìzšï°@œ¶ü%?ïã_0пÔ3Éü7ôc¿ßƒ~O;R¿Ù*ü˜lrð¿Ý|¢gô[¿ç\ß¶´]AGNbllSDSS J112405.35+204553.7?ïÿ3¹ðÁô?tڈ#¡«?ˆÁçÁs?tڈ#¡¾?ïû¿ŸD?YȨ)ž^?A'ï¿åY?YȨ)žd?ïòÍ
mÁ¶?d/'–±#c?Zeë$|'Ø?d/'–±#_?ᆰð¦æ?h½Yƒžq*?€UCÖy†?h½Yƒžq#4FGL J1124.4+2308?îC»#cB@Q{€Ü3rÀ:ã¿Í
	nÀ<]RÁmóù@T1I#4@bÁ–8?ÆM8`C¸?A±=é/Z@È1ÉPÁd?æcq>†£s¿ì>!£¿¿çà¾áý‹‡¿Øˆ¯üÝ`Ä¿ÞyÌÑý8¿ðAGNbcuCRATES J112431+230745?ïý0·~ìN?3½À‡"ÕK?6zD™?3½À‡"ÕC?ïü?×
Ë?b+0Åü)??NG'ª?b+0Åü!?ïìhNV?ooÈÓùû?cã—ﱩ²?ooÈÓùù?ïã'-ðÄ?X#ø]žˆ?lnÒ;÷9?X#ø]ž4FGL J1124.6-0809?ÝkL Ü>@Hv <K	êÀ;MFÚ°À<tò ›ìZ@ AêÜs@…Ù ð¥ð?Ï?8ÇǪ?£&Î 		ê?Ք˜B±@‰;¿HÕ²¿âBRÑ^,¿æbP1ò¿èð›.£¿¿cŸŒ¢»+¿è=…Ò<xV¿ïîåüH»[AGNbcuAT20G J112437-080643?ïùJß$€ß?EˆmÀšVu?Jԃmü']?EˆmÀšV?ïûâ¦Lã@?_¯äòXè6?@ufÌrþ}?_¯äòXèA?ïќ¸v&?|ºwd©n<?w1£Äÿí"?|ºwd©nA?ïÙ®ñ¶¾?`†›:xóg?s(‡x$ ¹?`†›:xóh4FGL J1124.9+2143¿ëםy¨RÓ@QgÙŽuyÀ;
)Ù]ëÀ<³ó;Ì_@r,…o7@B\=îx?ÆÝ«Â;#m?¥ùìj¡ßc?ã|楻æË?÷¼¿øÓç¿íxmÏç3€?ïú¬Î)Ä¿å{ ŠN£¿Ô	.3ð¿çnýäœÍ¿ÆjVJpKAGNbllSDSS J112503.64+214300.1?ïøŠÜ"?MUÈbhA•?O·Ô±\?MUÈbhA?ïש??ˆc'už?t+§§à ?ˆc'už	?ïØɟGfÃ?w]Àô6!1?s›0\Lžˆ?w]Àô6!?î0Xïò5+?šbÎV¥W?¬úqÜ­D?šbÎV¥W4FGL J1124.9+4934¿îri»ëÀ°@Ož@ÈG,À:ыxn§À<5ÜF½S³@ò5#ù.€?øNŒ¥•P_?¹ÀÖIxD	?Ã-ÄßB›0@)ÃÂb@
'AÜCb?ålk˜ÕN|?ïÝ`='l¿ÍüÖö¿Õ]°ŸÅ'¬¿Ôbºõ8§¿å_ü?EöAGNbll3FGL J1124.9+4932GB6 J1124+4933?ï÷ I"?IäàþÛ Ì?QƾálÚÝ?IäàþÛ Ï?ï÷n;'ß?dG'íFB?Q#ˆÞÚBè?dG'íF??ï‹çi‡?Š©‡ïãn?%žÿÜ?Š©‡ïãn?ï¿­¸5KÏ?mÓañ	4Ð?€'ò­©?mÓañ	4Î4FGL J1125.0-5804¿ìpBMè"@ ñ,'¦7À:M¼)çZÀ<zF"b@!þ"à$Œ?÷';ý?ÆûQš|m?Öw¦)ÊÔ¥@‡‰Fe?@K'à—ÚÓ¿ïýVlô!¿ï+Bn9™?ïýÀTïEž?Ð/ûZԷӿ͕c>"¹†¿ãϺ 9qAGNbcu3FGL J1125.1-58032MASS J11250388-5805404?é,¯¯¬î?¿´f0YŽ¾?ËMAALG©?¿´f0YŽ¾?íÝL‡üÿ/?ÄÚÓסF?±›ÀŒ?ÄÚÓסF?递Ñ£?±[nùu?Éýµ¼»¹u?±[nùu?î–h}çv£?š/ðæò®¨?¦™x!ˆ•Å?š/ðæò®©4FGL J1125.1-2101?ål¡©)¥¦@BÁˆ†aÀ9îÚøººÀ<:¿:=°@u,ŽSj`?ü©—"ÆÔe?¾OÓ@É¾?Ä÷'>]@Ôi
à"S@Þ跎ø¿ïòx6?ï>Áï#9¿Ò´ßñÙ¿ÝÑ·D¥¿ä¬;'}E¦¿Ýdæßr–ËAGNbll3FGL J1125.0-2101PMN J1125-2100?ïöN¤"Ѭ?P­"Œ?Sb¶Ø\¨Å?P­""?ïö9aö0s?f7'sƒ(?S<Ÿþ?f7'sƒ(?ï°yd"è8?'`0TrË?ƒá¦ÛòB?'`0TrÉ?ï#:om|Ö?ˆ6çc?›˜²Pe+?ˆ6çd4FGL J1125.5-3557?з½e¡¶@7¾ÕϪ͟À9Ý¿zÔ²tÀ<:b'œOV@"A"ßÿ@ñÜPÎO?²ãÂË O?'B@c®Œ?ÒÄ«Á}œ@.~]Ë?ïÿ"g3¿áß
Q'™Ë¿à¬1¡¸¡ó¿â7´lƒ¶Ù¿Ùˆi[
lпßr&c$ÚAGNbll3FGL J1125.5-3558PMN J1125-3556?ïþ'•Sg¨?"€{ÆÇÜ+?&֪Ʌuð?"€{ÆÇÜF?ïþSMS=s?B+Gö
%?*Ë*Ì(É©?B+Gö
,?ïó±-)æþ?d•®ly?X¥¬2N?d•®lv?ïýç °|K? ËZ†B¥?0Æú|«ú? ËZ†Bx4FGL J1125.9-0742?á_o‹k@H¼ƒBÙÀ:"CïCÀ<_^4h½Y@ò¿ûƒ@ÖqáÄ«–?¿cÌ®…?`†K¤«?´É¼L!?öå§×ŸäŒ¿ïÌ7å?ï~•Òd¼B¿ã…Lò!¿â¾œ)¥ì¿ÙH¯œ:^¿á¥·]®1AGNbll3FGL J1125.8-07451RXS J112551.6-074219?ïڌ&P¾?pÙÄÑH?r¹ì× ý•?pÙÄÑE?ï×ÏJ~?ˆ…#o•Ÿ?tv˜Zõ@»?ˆ…#o• ?ï¹J†•zš?€µ!7•?­^Z¡Y?€µ!7–?îŸ jh>?•ª‡#M»?¦
ù_¹|?•ª‡#M»4FGL J1125.9+2005¿×âu´0¦@QNµ ÝDÀ:ÁóTöÒÀ<m2ûÕÎÔ@ØdS爻@Âãú滋?¶h#ªÕM?«¬d!'¡Ù?ó¶îßFL@î[R×é?í.öWà'¦¿'ù†Fß,¿æôxþŸ3¿à2üâ>N¿æï¡ðÖ¿ïÿþÐñAGNfsrq3FGL J1125.9+20074C +20.25?ïü³7sé?;DÜåܐÖ??¢fD`°ä?;DÜåܐ¦?ïý~~€çl?Lj3Ÿ¾?4øęî?Lj3Ÿ»?ïÄ8¤†ã<?X´.ørT?}ã­¼ŽaÙ?X´.ørT?ïø¤OºË?=D3§¶[?MnÁˆÕ'?=D3§¶[4FGL J1126.8-3829¿ê3\Y{¯@5uX!)EtÀ9¥Ìô9ù À<>ô±d¡@÷oV¤ýP@|½ÀÀO?²Êà
œJÏ?¶˜ã¼'Ž@aÑü·v#@8³Ík-?Á4âö.ðÙ¿ÝEÓÿqá¿æs	¿àwy¥Œ¿ä3ZÖk®¿ïüev|^AGNbcu3FGL J1126.7-3834PKS 1124-382?ïéñÿ‹Ø?b>âEfáú?ft'ñ?b>âEfáú?ïÓºKþí?Š¾MÆ?vw"ÚˆÉ?Š¾MÇ?ïÅ'Ñûš¹?Ày€â"Ÿ?}l2£f?Ày€â"?î¨Ö4MÌ_?‹º¯mÓZ?¥rœ»#:?‹º¯mÓZ4FGL J1127.0-1857?îã9bkh*@Cɚ¿3‡À7s;dZ¬À;Y–¹‰$@vú«Ø5Œ@¼ô}þ•?"ÕÊCÒà?´ägH8¨é@!ŽGUÿç@ "ŒdQä¿Å`Ó)ˆ9 ¿Þožˆì£,¿ã‹à)÷¿ãèJ®kc¿æy2Pµ$:¿èžÎÂpRxAGNfsrq3FGL J1127.0-1857PKS 1124-186?ï÷Êfš
?MLéÒt6ù?Pk3ÖËëÄ?MLéÒt6â?ï쐀ÉNŒ?x̬…!?co6±sâ?x̬…"?ïÔÝõJþÆ?{˜5H¥V?u'Z€œÌ?{˜5H¥V?ïÿfLµ?2&Ú*w[?ó6i\)Ò?2&Ú*vÃ4FGL J1127.4+5648?êRóәAq@Lbك"t—À:KÝþMxYÀ<ªþÊuÚx@
ÀaÖ	@mñf­´?¹A]˜a‹5?´ü‹+lÀH?õÈbŠ8ӆ@/Vôk!?ïÿäA2¥D¿è"d
ƒ ¿é3)Wèb¿êSi©¿æ€››ÒXþ¿ïÿþªJlAGNfsrqS4 1124+57?ïÿÌ$ 
à>ýu|͓žþ>ùí¯ùz&>ýu|͓Ÿ7?ïý7y6¬Ó?Pn_ƒ(dÞ?6D6J™^8?Pn_ƒ(dÛ?ïÙVvHJ?vÆ´"=?sTÄò[Úç?vÆ´"C?ïñ;Hæ
¨?M"úëØ@?]‰n3ê°?M"úëØ64FGL J1127.6-4920?ï›wÃlM¯@&Mv«XÀ:^ȋ­À<K€\±±¾@
P_=þ@@6m
J?Â_ý–™4?ÀÚÙÕÉˑ?úZë=Ñç@p
«T­¿å´d@q_>?ïû2¦Ey‡¿ç€"Töοâ¢+¾Ê«Š¿åÃà‡ÿå+OnÓrAGNbcuMRC 1125-490?ïg
™Ì?™3:–r=Ï?"þLÆ}7?™3:–r=Ï?ï$áTŽ\Ã?®ÚììØ`?›cÕn4g?®ÚììØ`?îᫌέ?œ«Ä©¾R^?¡åG3å-?œ«Ä©¾R`?î¸}½îG'?'V²U;?¤x$!‡Ç?'V²U<4FGL J1127.8+3618¿ÓˆAÁ!Á@Qƒk¹Œ~(À9m©PÇÀ<!gÝ^ëH@PÚqÐý´@в\Þþ(?¥·ÿʧÑ?¥õØ£‰vP?þ­üwµCC@侬ùrÈ?ë^Ɣ¤gS¿å®É¬†Ü(¿åøq–EQC¿â=fȋõl¿è"‹BhÛ6¿ïÿü¥¬¨AGNfsrq3FGL J1127.8+3618MG2 J112758+3620?ïüÁ	Z?1%jsV`¢?9÷'çµ0t?1%jsV`~?ïû´UÚê­?TÇ×F†ˆA?A.¨"UJ'?TÇ×F†ˆI?ïÔdiã]?uÁXÄ¥Û?uÍòËQH?uÁXÄ¥Ø?ïù±dÂÆO?<­½c¶:Œ?I:lôæÄ6?<­½c¶: 4FGL J1128.0+5924¿ïÏVËÚ@KU¬îàóËÀ9æ±iÀ<–[žŒG¡@ÎPV"œ@T¤°N?´ŸÈêTó?¶r:@SéG?ÿþÊuÚx@ªÂ»{싿ÒÐǘ°eŽ¿å¤ "ˆÞ`¿ä¤{(߿傚Nʓ¿ï¸Ê·H׿ïÿÿ" 5•AGNfsrq3FGL J1128.0+5921TXS 1125+596?ïý»PÇ/O?-eI $5·?2%yƅ"?-eI $5¾?ïüUhÁ(?QšQúµL?=T¿QöÆr?QšQúµL
?ïËâÌU½?zñï£ðn?zôÕ!˜?zñï£ðl?ïõ®Ä°QY?H¯<£?T¢vŸ]O¬?H¯<‹4FGL J1128.8+3757?ïWŸ·ê¡k@Qd~¡ÆÀ9ψ*ÜLÀ<	óˆù8f@ÂQ} <6@?f"‹?¼ÚeÐÝ©?¼Fí¥4'i@£ÂÀ®@½Œ¾)q?©×•	'ú¿×®sûû8›¿åì§]§{¿á'Á(SÜ ¿ê²œÕŽ<n¿ã_gÍAGNbll3FGL J1129.0+3758NVSS J112903+375655?ìj·9:?·
IK¶bT?¿DªF6/ö?·
IK¶bS?ë͝<c?Ç݊<DNˆ?ÂÀɋt?Ç݊<DNˆ?ìŠÉXÒF?¨†í¢¼R?»©·%9mÃ?¨†í¢¼P?å;\])CÝ?´Ôã?ՉGE­xF?´Ôã4FGL J1129.1+3703¿Þއ¨ÖÑ´@Q€Ÿ¸fäÀ:<‹FðYÀ<`'o@á'C'¥.@ðäFfß?¿*^x[[p?´1 ‰Š?ö¾aßîé@"§×Êת¿ï ˆ!ö?âCbn_.¿ä›ª€qªg¿Þ³æ¡à¿æÔÎùÍ·¿çÁšÕü4AGNbll3FGL J1129.0+3705CRATES J112916+370317?ïü£ŠªÍD?8÷©«-ç·?:㪩•Ýa?8÷©«-çÍ?ïüJÀ²û?U`k‡kä?=¯úh*ç?U`k‡kä?ïéݛ|I×?qrËçuxÒ?f"dƒ¶(ð?qrËçux×?ïð<8o¨¹?Q¤A3Ø?_‡ ®Ž×?Q¤A3Ø4FGL J1129.2-1014¿ÔâÚӕ—?@GÑn¬†hÀ;9ÌýpÀ<¬Ök±ÿÂ@âŒXhvâ?ý²—a°õ?×5E2E?ÊQÈà5j?ò=0ýÎÍX@ÍîµÕº\¿ïâЯ°\T?ïgÂâ=Lg?éííÿL{Ú¿ÓVŒúk¿æ'4JŠgÍ¿ë#à¯Ø @AGNbcuNVSS J112912-101349?ïó0^´?SlJ¬½ìî?YџïB——?SlJ¬½ìï?ï÷$Çï"?u•AùnÔ?Q¶q Úh?u•AùnÔ?ï lê'$'?ƒ
"Ÿ+ö?‡äÅ[¶Û«?ƒ
"Ÿ+ù?ï^Vä^À\?"K#ôÞ?"5#t'ô˜?"K#ôÞ4FGL J1129.2-0529¿´Ô!J¥´#@IçiüóÜÀ9¢š4Ê(À<$Sœ_G@;°É6@ÆX>…w?¶¦¢@²!Ñ?½2XíW\@sbb˧3@c¯˜	?ïzÇw"¿èhǍè¿ç"F{åS¬¿çhÁ?O÷¿ïÿülò¿ï³½œ®!AGNbcu2FGL J1129.0-0532NVSS J112914-052856?ïø¢:ùÔ?XJu2B.ç?O¡w´7?XJu2B.õ?ïöÏÿÁÊ?pØüÃm¨?SØ`|jK?pØüÃmª?ïLñÑF'?†*'¨Ä*?ˆ¬Ã‹®["?†*'¨Ä'?ï_:ÿ#>î?€.ä1b˪?" ˜"b?€.ä1b˪4FGL J1129.5+3034¿çzcDž2@Qð¼¾aÏÿÀ:¾ƒ""^ŸÀ<•È¥i±@«*"ýM@<§P;¶?Åׄᦣ˜?²Lêi?ë̘"¶ÛÊ@íØ>šð\¿Ý"±ð)É¿ç©¿+¤t¿ä£TY©¿âÅõåÊË¿ëýØ"kdÓ¿ïó ‰ƒœAGNbcu87GB 112657.9+305242?ïûW
3*¶?<—P‹£€?B£×3U#a?<—P‹£8?ïü»f×Y?VÁg¼²Ö??J$ÉE/&?VÁg¼²Ô?ïå°Vô¿?sLh'Í?jýO©@U?sLh'×?ïèíŽï‡?Vˍ2"¾^?gôqx'?Vˍ2"¾^4FGL J1129.8-1447?Ò¾P³~kØ@Eє[l7aÀ9qÈÉ2
™À<ë˜iî±@,ZÝFA®@<bÿ©˜ë?²ýáÛ¹¥?ºWA°N'Þ@ƒ¶æ±za@
'õèO	¿Øƒ´?3°¿æ'Ž¿éŠ¼‡k ¿é+'Ëöä¿îC+κ㖿ï°ÿ|L¹AGNfsrq3FGL J1129.9-1446PKS 1127-14?ïý@ŸiÜ-?2…¯û8|™?5û±™E?2…¯û8|¿?ïýCë(hD?RzY5œëÆ?5়½ãP?RzY5œëÅ?ï¿äEpüq?zx¤ G—m?€î£Àä?zx¤ G—j?ïÿŸ!*/m>ýþýÆ)àÝ?7µt$†´>ýþýÆ)à4FGL J1129.8-4217¿Ð4r"õaü@2˜ú7iÀ:Ç—×øzÀ<¯¦âWx@Å°ù³@"`št‹?ÉGHÿMR™?á|â(ԋ@öOv_Ù@'·þ¯¿î l¼Á¼Î?îPz×6³¿Ù·]d_%*¿ãä±i¿ð¿ïpêÄ.™AGNbll3FGL J1129.4-4215LEDA 566417?ãm'
ˆ?Ë|2x«^ë?Ù$ÜýëÐð?Ë|2x«^ë?åâÚrì9
?Ö[¬Z?Ô:K'å?Ö[¬Z?Ðýtz")Ÿ?´Ù	P(5?çE½ë1?´Ù	P(5?ä>'q´­?µ'Ì¢umÔ?ׂÛÛ–§?µ'Ì¢umÔ4FGL J1130.5-7801¿ïXØxôÁ5À/¨'ÿ'À9ÿ_,¶ApÀ<…I€|'@!Gø%ÁÃ?öŒ©[®|€?¾ ﹶÅy?ÅÀµ§Â&V@	‹)CÆ(n@RҵſÈp¬æR"Ý¿ïÿíáoq'?ïÿo¾ÁÇ¿˜ìû7昝¿Õ‰ yݒ¿ØÈ\ûƒ™}AGNbll3FGL J1130.7-7800SUMSS J113032-780105?ﵺëÝñU?~Â/Ô"¾!?''Eƒ«
?~Â/Ô"¾!?ïô 3?v±U‰Ï?Vü¿Ùۛë?v±U‰Ï?º'¸Ý?œêa"ö?¦d"VÔrG?œêa"ö?ï¸ù
˜
£?qËK4Àë?Á½YýWu?qËK4Àê4FGL J1130.5-3137?葽%I@<+-À;œ%¸÷,óÀ<ÆiH˜ö@#ÌP×H?õ~z#²Œ°?ѓa^j?µ|ã«`–n?Þ¢èB2›@e‹-m?ïךÈÙ"¿ítÎ6/g¿ïù–#?ïïšø>jŸ¿Ü®_¤U_¿=aƼàAGNbllNVSS J113046-313805?ïÿb—æei?¹/-;?­3RÞj?¹/-Ê?ïûlöڄ?ddrd¬¶y?BMÈ$•òè?ddrd¬¶{?ïë3ó«íl?hƒ¨0ž=?dÌT"¡?hƒ¨0ž;?ïõùˆ2?Rƒ®Ü Ø?Tï›Õá?Rƒ®Ü Ô4FGL J1130.8+1016?éôBö%3@P'»ƒÏ,ùÀ:e$Ã-çšÀ<b(Cëè@áðusu@Ëeè'?ÀÏa<0?¨?ž)\?âùâå=@s¦¸»ó·¿¾Ä(cvq÷¿çË@Fìù¿é%ØÝv¿èO‡A¨@ü¿ïâöý»'¿å§/^½O¬AGNbll3FGL J1132.8+10152MASS J11303636+1018245?ïÍÀ«fhÕ?x!êŽøä0?yªL˕¹?x!êŽøä3?ïÅá†ââ'?'0;¯•žT?}<ŽŽì{?'0;¯•žU?ï‡ý%û×ä?†-ÒMPfó?Ž¶
µ?†-ÒMPfò?ïKsEÉ?ŠMÔÿ§j?v'ŒWFá?ŠMÔÿ§h4FGL J1131.0+3815?­¶ÆĜÂ@Qtw—|À9/ͶígÀ;Û£ûkq@‹D¤bË@d[Ëر?¬yð±ÙVs?ļ3b(¤@Š.Ýc@6c¿B ?íWZYè©¢¿äX·¼šO¢¿ç?³ÖhW¿è܀žöѿꦭj0ö¿ïÿî' ÇAGNfsrq3FGL J1131.4+3819B2 1128+38?ïÎpÕ¥&f?v•¼Fªí^?xǕ-lÌð?v•¼Fªí[?ïÖ»¿Ÿ D?›z>Eh?t¢ 0/ݽ?›z>Eh?햝³©é•?¢üÍÚâÊ?³Kb°³Z?¢üÍÚâÊ?î*áp<ë$?•Ç;ÎïE?­Qèü1MÓ?•Ç;ÎïE4FGL J1131.1-0944¿âˆºÂ	Gí@H(A*2À:Ò
¨y0À<‹Cp˜@ ;øå¯r@"÷…zÿ?½µj/ž©#¿¨0€Á"Ö?î*käT¨Ï@u<Z#?ïϤMQÂj¿èZԂ"Úv¿â7}DÏ=¿àeòmpEã¿Ù˜,F¯çº¿Öç`Ÿý·AGNbcu1RXS J113104.6-094353?ïöz<£#?IÝ}eɆ?Sù†¹ºI?IÝ}eɇ?ïùÑÌ!+Ë?nq!è7ô?H¸Ï{PÍø?nq!è7õ?ïòÄý1Í ?h¥5Ã?Zvœd¾¡?h¥5Ã?ï¹l­}¦?j²kxr'%?¤Ô ˜–t?j²kxr'4FGL J1131.4+5809¿íϘ4'º•@Kú¦">jÀ:}mÿ·Û¤À<²bÒ]/†@P1ÏZñ"@M••_?¼´È?œœà²'?âa…V¶K@þ•dU¿û¿ïqsªò‡q?ïõµú"pm¿æÇ1¢a‡¿ÑT‹<߄_¿ãí©¼&Œ¿ä½öp4E'AGNbll3FGL J1131.1+58101RXS J113117.8+580911?ïý° \?5"Òe­ü?7êýƒ?5"Òe®'?ïûï˜H'?UA_ëô<?@AŸößdÅ?UA_ëô.?ïóÀ*ñR?`<)ª>?Yþª^;?`<)ª@?ïæJ5*?\ج!'`Á?iïµÊÕq?\ج!'`¹4FGL J1131.4-0504?×"äg¼j@J9Wÿ›V2À:¡›Æš"À<H­œ…Ý$@ˆsü|@¶ð<=ð?Ê-ë˕•(?ãØYÞBÀð@cì‰*¶@	ùBWC¿ìŒòãÕ¨?áœ#íEY¿æòŠêÕ¿êw»ûS¿è«ïxÉ??Æ­°½L§#AGNbcu3FGL J1131.9-0503PKS 1128-047?Ø}ÃÝÒÐý?Í¡.œ÷û?ãÁ—'?Í¡.œ÷û?àï
 ;¢?Öþ8¸ñ †?Þ!ï俈»?Öþ8¸ñ †?àkÃïã¤ñ?µ¾9ÖçL`?ß(x 8¶?µ¾9ÖçLa?ݯ¡¢v?»ðùё÷?á(/.ý9D?»ðùё÷4FGL J1132.2-4736?î+"†Š¼@*R¥'ÛçóÀ:&vŠ ØRÀ<K½¹3'Õ@ üSøû?ÿÌð©Jç…?µc+Ì¿J5ÖD¨x?–Ló½kI¿@"NÀ,€g?ïÿò(¦è7¿æ{B`Í 1¿ÞžáIå¿Þˆ£Ós¿ã3ªò‡qy¿ßÝ~ ÄÜAGNbcu3FGL J1132.0-4736SUMSS J113209-473856?ïýraA?6æ+ŒB?7ŒoÌõþI?6æ+ŒAÜ?ïûØ? ‡-?_µb
c<?@Ÿ}ãN$?_µb
c;?ïì–yǍ?k&56
ê}?ci†8rå<?k&56
êx?ïÙ/gþ"'?`ю BM?shL?`ю BN4FGL J1132.7+0034?íזr'+@Lµb8Ú<!À8j¬=áÀ;ÎpmP@–Eý`@åM|Š•?ž±ç÷©"?™­ƒþŸ$??÷¹÷2ú(@	á þ'bÅ¿Ñ:b|vóý¿áX»]c³Y¿â¨B(ïb¿àíàBËV«¿ãÜU•:¿æµ£ñpwAGNbll3FGL J1132.7+0034PKS B1130+008?ïû;-
³?@A;'ó³F?CßKÕ8Ý?@A;'ó³X?ïìøÚµ›•?‡°ˆù6?c%JdjE?‡°ˆù7?ïƵ!ÖÇ?"Ä6
"d?|ø%oœÜ?"Ä6
"a?ï›Í|%
«?{9D™Þ?‰ ö¼•c?{9D™Þ4FGL J1133.8-2048¿ïòIÔcúz@CA3 @|ÈÀ;J¥»æË|À<¬.î*§@ #áÜ~q?묔é0°¢?ä#²VÿÁ?í'I†\@¥#±µð?úÚ!nºË¿ë<…ÂL@?ïèq£±J¿æ­—}_§?ËHvü¶Ÿd¿çù_!£"ÿïúDÕ&§AGNbllNVSS J113350-204852?ï'=u3…Y?­TåH?‹°¢³©¬?­TåH?ïŸþáþ?ªÕAaI
?ˆ<y€G€»?ªÕAaI?î{
Ša…?™´šÆ">a?¨O&'Yç¸?™´šÆ">]?ìŸÐxO€=?®zâіá?»|=ƒþ?®zâіá4FGL J1134.8-1729¿Âùé՝=@DÔ€À;Wc$'†À<¢Y …F%@" Ӊ)‰ç?ôÁjî‹?ä),~ä®?ӂݕqì¬?üýî'ð2-?úkQ'n×ú¿ïƒŸâˆö´¿ëÓÂõ³uä?ïúgïÓb¿åfc á¡ñ?¬Dà"º^¿ÛUü wnÌAGNbll1RXS J113443.6-172853?ïïÛ9¯Ž?c6,¨"å?`$ñÆPqž?c6,¨"å?ïûøYí?ULæn©¨?@³¾˜WP?ULæn©©?ï\óæaÃ?"iY?œTaƒ3Ç?"iY?ï´ÛÂ}â°?zÙ€5ýM?'É`‡Sï?zÙ€5ýK4FGL J1135.1+3014¿ïþSlûŠ‡@R@I<‰ô
À:ŒNrSÚsÀ<^6=@IϚ¦ã@ôQƜ1$?¿7)!Œlµ?†æՕ%õ?ËoY­€@_²ïyu?¼˜-žHÕÝ¿ä©Xž§ m¿æü­e(¿ß¦+xSδ¿àï€ô‡&¿ïø
ÞpAGNbllCRATES J113514+301001?ïýg±w>B?.š³~[?4ÂtF
ã>?.š³~,?ïý®$Î1?MÉÏ~ø'?2ŽÛñŽ|ö?MÉÏ~ø¿?ïð'?Þ+Ú?e]Ë~K» ?^݀C¨M?e]Ë~K»ª?ïýF¨Ü
n?(FP$¾ñµ?5ʹ"'Ç?(FP$¾ñ£4FGL J1135.7-0427?ï–Ã/²Š@JÀI¡3ÁÎÀ:Júì.'À<'cXK@4¥šõÿ@´£@ˆÊ?Êóˆù8e¢?ւc€Wÿ@<»r1v@p8²N¿âÉäà"Õ»¿ã²['ÕÝ¿çéüÞbvm¿êTÅ¿'Q§¿ß^?cR¿ïÿ‹Á>ÏAGNfsrqPMN J1135-0428?ïæ ò܉o?oÙQ?~yA?iß
#v'
?oÙQ?~yN?ï÷aV**V?ið{Vm?Q=S««T¼?ið{Vo?ìÇ"i؝?¤ûd£Öß?¹ÇÓd±;?¤ûd£ÖÞ?ï}ÿèó,?|ŒY§¹ô?@ýašz?|ŒY§¹÷4FGL J1136.0-6824?çU;ùUiÀ3wÀ*ýÛÀ9ßzR÷À;Ý=ïí™@À¤[>•@7Á•aü?ÁÜæujeO?Æ9,œk@þ|Tå5@;BÄÕ?ïó˜H`Áâ¿Ð'¿ŒÈP¿åú!ßxËï¿èûYbFò¿Úa3ÁÎl	¿ðAGNbcu3FGL J1136.6-6826PKS 1133-681?ìÞðÍ´?µm¤Žiùw?¹‰'_Ô?µm¤Žiùw?ì®È'þµ?ÂDi'Å}À?º‰»èšR?ÂDi'Å}À?è¡¡µ´?µØ¡ÿ?Í{­y)/®?µØ¢?ë.—=ŠTG?¦àvz&Œ?ÃE£	Ö®æ?¦àvz&4FGL J1136.2+3407¿ì˜Ä\A±@Rûüe@ÌÀ9犰ȊHÀ<}Mæ<à@¿8Ëùh6@ÝGËÂâ?µs[|T?¾w¾}~°à@.¾`"€@Ó×½k°Ó?ÖùXD¿ä´Ò9ô"¿æ{{*·å¿é%ãõ~z¿ç`…¡j€¿ïÿû}º@AGNfsrq3FGL J1136.4+3405MG2 J113627+3408?ïþÔâ5Oº?!
¢zˆ?"±Ü«C¶?!
¢zˆ?ïüFIÇU?U®f±Ï­?=Í·!ÅQÄ?U®f±Ï­?︈yŒ6o?}ï˜'{?Ýáœòcê?}ï˜'y?ïýÐCây†?#͇ÇÑ´?1}àì3ÌÀ?#͇ÇÑÌ4FGL J1136.3-0501?ì4¯Ù³IQ@J‰¡ÎòAÀ:…0íÕ·À<³çcQ@Íe+'öê@º=c7ݽ?і]çM?Ýî~ƒÄ~@r+EþçÒ@'rÒZ€?ã'ZS<=¿âқ®FÏÈ¿æ̀÷Œ>¿é¦zÞB•ý¿ïÿÝe¡D‰?ïþXËs0yAGNbcuNVSS J113607-050156?éq³1¯?Å;Û›]Š?Ê93ƒ«9D?Å;Û›]Š?ã0Áº!vG?Ô:*MZ§é?ٞ|‹½s?Ô:*MZ§ê?äT¶€–¶í?µui®?×V'þҒ%?µui®?Þ±:è¨^?¿È"múô?à§{⋫Ñ?¿È"múõ4FGL J1136.4+6736?­p]ËHO@Gú">iƒÀ9ÊÛ-¸ŸïÀ<Td«{Cm@ o@)»»?ûB%YUÜ«?¯bJßž? –´6þÄÂ?óišÐ@
"M'ëð?îŇ^-³?ÉO[¹¢¿áµR\Ä&¿Ô.ÁÙ©ª¿Ø1tí¿Ù«¨$v×ÎAGNbll3FGL J1136.6+6736RX J1136.5+6737?ïýûS@f¸?&å>ºõÛ?0%eüÊHµ?&å>ºõÛU?ïü*¦?6§?V=cÍhxò?>ªÎJÁ¹?V=cÍhxõ?ïòŒvoG?eõÚ1Ý×?Zçé!ræ?eõÚ1ÝÜ?ïî¥J&e¤?M4×	Hœ?aZµÙš[A?M4×	H"4FGL J1136.4+7009?ïùi$sú	@FÒ·`,'À9¿¤EÀ<	?öå@x{‡µÁm?üÕýb–Î
?¢cŽ"u©X?yÁ"KùÕ?؛Øc-÷µ@
Ãsٖ‰Å?¤A_r>¿ØªÀ2Š—¿ÝžN¿Öš+¿Ù¦_$Ӟù¿à=At>–>¿ÁÃõãœrAGNbll3FGL J1136.6+7009Mkn 180?ïÿ%ˆ7ðú?F©ñš?Nùà¯Ò?F©ñ£?ïüh™Õè?Tñ‹}äQ??Ü»1P¾"?Tñ‹}äQœ?ïô®Ø'?d÷ÿ6€''?V¢Oé±Ô?d÷ÿ6€'?ï÷®øü!?B›Ÿz?P¢Á¼q?B›Ÿ¤4FGL J1136.8+2550?ë é±ð›y@RQõ@‰]À:¯Q=à5_À<–/#ÙùÜ@ ;%Öÿ*Ã?ÿÇP ©Ã³?ºf¨UŸß¿£Ù,"=Š?êTø³¥@oZN€?ïôÜJ婭
å¿×Fb$S¿ã)ªžNµ¿Ü­ž^Ok£¿±!`ÍË$AGNbll3FGL J1136.9+2551RX J1136.8+2551?ïü9«Ü$?:AÅ<¤!X??æ2¡Úÿ?:AÅ<¤!U?ïüúԄÞÆ?PÃ`RÄÉ?8)[Ù	Ø¿?PÃ`RÄÏ?ïð?4íQ?i±Ó‹á(?^偖%`A?i±Ó‹á("?ïÔ¯¦C–?b÷n+‹w?u¨,Þ4üÆ?b÷n+‹~4FGL J1136.8-7413¿êgvœ`À(4¹#¢œxÀ9zŠ‡¿À;ã5ÍAfÓ@Äù·;–@%Қl'q?³z&P Õ?ÊËí>\\!@=s!_Ì@‹ú¶j	ß?ïýaŠ^"3¿Þ
üGä› ¿ã4ýØ"¿æ¦ãÏGÑP¿î:ò¥µ1¿ÑÇÒÝ2¸AGNbcu3FGL J1136.1-7411PKS 1133-739?œì!&¿3Ò?ŸŠ±àOñ?ïžöÊc?ŸŠ±àOð?®Rvo(Ã?³ËflœŠÂ?îؙ
~¥?³ËflœŠÂ?Ƙûí–¨?²5%Ė£•?êYÁš{W?²5%Ė£•?ÁÅôf¹ž'?¢±#¥Pe?뎂æQ˜^?¢±#¥Pe4FGL J1137.9-1708¿è²ÏUf@E"_ !¸À:–,Y$^"À<CõwæÁk@ ìç¢fé?õÂFçE?È(éè‹Ð?Ñs}\º@	£qÚ7ï[@)£šyhw?ÓP¯°\S¾¿ÞDÔÛ¹ú¿Îì%'›{?½e)$'"Í¿â6o]…í¿Ô?·¥ôïAGNbllNVSS J113755-171031?ïÕÎ1 ó?t/wí+J-?uç9/…â?t/wí+J-?ïú*zp2æ?]CõÀïQ'?GV?4hK?]CõÀïQŽ?{Œ?›î~5?¤†nXG?‹?›î~5?ïÉV?fùŒUsñÜ?{»©Tñ™?fùŒUsñÞ4FGL J1138.2+4115¿°*ÖH¿Ü@QXŠï²ªãÀ;`OËð.À<±§ðtqÂ@ 4C(ž¯®@,ZÑÝ®?½F‰§357¿¶dù(öC?û{
¢ò)@ÚD…ëçÅ?ëçlU"°L¿èùŠ—ž¿ãù.ŠWw¿åÛWª¿×ÙôhI¿Ý¯çä«:×AGNbll1FGL J1138.0+4109NVSS J113812+411353?ï÷/ÀlW?Rà%‡g^?Q¡'Si?Rà%‡gN?ïû›¶)K?Tù.x=<I?A"'ZØË?Tù.x=<D?ïÞÌoÔÉ?y‰bN=?p™Èõ?y‰bN8?ﻝÃ$"í?nûà›ëU¿?6ÚÅ:?nûà›ëUº4FGL J1138.4+4857?ïÁG·ÉJå@P†­-ËÀ:¬¸ô¨´À<¤k'QÕ@€šˆÕ@ÛçòÛ?Ào\¯-€¿¢3NSÙØ?áz‰hÉíõ?üâf´êØÑ¿ÙÚW¤×J¿ì`¯7¿Û¨üct¿ìåvã)Û¿ï÷³•Ä"?™A_(…AGNfsrq3FGL J1138.2+4905GB6 J1138+4858?ïïàáTG.?d›r0ýY³?`«¸Ñy?d›r0ýY±?îÓ¡ûxˆ?´]ú°CôU?¢ÅàHw~Ï?´]ú°CôU?îë>Ù˜ ?•€oæ$?¡Ln&uù?•€oæ$
?îoœpãzÞ?9a®
ðü?©8ñÈR?9a®
ðý4FGL J1139.0+4033¿ï""H‹Î@Qzµ^ñýßÀ:C¬­r"rÀ<4cʪ³@eMÌg@ŸžEÐÄ©?Átˆhî?µÚçÜr²?ñ¦+]{Ü@Á¿M2bÔ¿ëv_ß
¿ԕOó]ZN¿èƒ_›q
.¿ê"ö^ìtˆ¿ä˜íÂeÀ¤¿ðAGNbcuCRATES J113903+403303?ïÿ}Ž¸¢ƒ?FRPE4?N(믩û?FRPEº?ïüŠ….Wº?TDL˜ñÊs?;«ÖB0a?TDL˜ñÊ|?ïê?‰ºNgÁ~?Œ…y{ÿ~E?‰ºNgÁz?ïù«ï?@Ià!јù?KljQÀ??@Ià!љ4FGL J1139.0+5530¿Éƒ²D 6È@M_â?$ØýÀ;æéóN@ÖÀ=8C=lr@"ì¢$'–H?óÂ}qDç?Ög†aƒ}£?Î1·ÝýKÆ?öäí@	Û@gÿtißB?í!¼{¿ïÿð`OËð?ïú­EH­?™Ü8{$A¿•↦¿ÙsË©·AGNbllRX J1138.9+5530?ïõ©é¬G¥?P¹¨t?T¬,§pµ²?P¹¨t'?ïüµ^˓—?Wÿ¥S®?:U	£cWg?Wÿ¥S®'?ïÊP»x¬.?zÈH'óŒ?z×¢C©é?zÈH'ó‡?ïòžÕ³Ê?S@H– 'A?ZÂT˜kÙ?S@H– '>4FGL J1140.5+1528?ì̱8·õ²@Qu'·þ	À:þX;*xzÀ<†[3,}7@"«Hî†?ûŽîDì™?Ç#KŸÐ-?¢8¾Àù
?Ú'Â	Ð8@Õ̉…û,¿èÉN][$ê¿ïm"Ãqx?æ»ss•#¿å·¤ëàŽ¿"Ïюþ`¿ÓÏ-"óoNAGNbll3FGL J1140.4+1529NVSS J114023+152808?ïþ]¶‡A?&s.ruÉ?*$—Ó?&s.rv?ïþéMÌ4?F€]DY?.Ak#<¿Õ?F€]Dm?ïçì$Šú‰?hlL¨öO?hÛuv?hlL¨öO?ïë/0ð"Ü?^Éޛw8 ?dÐÏl%<?^Éޛw84FGL J1141.4+6805?êÂI¡<] @GÚ.	þ†ƒÀ:NjY¹À<Ž-ë˕•@ ÏU¢Hê«?öd»®²?Ãß\œc"?Ðñdûµ@èDŒ÷ʧ?ûº¤¦½ïd?ïåôñ¯e¿ï²¢´ËNH?Ž±ß¿È¼]¾ÍÖ¿âT,Ý®œ`¿Ïo¬ö˜£%AGNbcu3FGL J1141.2+68051RXS J114118.3+680433?îÁqµø§ø?£ç²ooö?£èä u€v?£ç²ooö?ìkNZï	?ËÑ=·'Íõ?¼¥(‡·h?ËÑ=·'Íõ?ì
0Uí¸Õ?¨¼ì푪??¿®}P'9T?¨¼ì푪=?è9¢³M…°?¼ ïy5?Ïu2ÉéB?¼ ïy54FGL J1141.5-1408¿ÙÀ«gÁJ@F°Bž
A¢À:žë¥ÕçÿÀ<w»dg@ y‰®¿ñ?þãM­1üÒ?ÁBÎ[ÃO?¡p¡æð?á±ý2Æ&@
;"ÇOŠ¿ã7a–5¿ã,o_3l>¿Öf9ð¼–¿áòʍWkø¿Ûï½µ'®¿ß¤õî.FAGNbll3FGL J1141.6-1406NVSS J114141-140753?ïÿ§ü›?øYÁü;?ë`lÀ¶?øYÁüŽ?ïýê8¢}?H«}
?0®:ï\o?H«|Ø?ïù€ØEW¾?bÕÐå?Iüžê¡L?bÕÐì?ïýfí9?#ÙNÞ­S?4Ϗ8–8¦?#ÙNÞ¬ô4FGL J1142.0+1548?ëŠv´Xõ!@Q"¿aª?À9˜€£ÿN)À<7€@,?ú@rŲ|>•@zãËìÓ?®pC£²û?†oHQaÛ?׏ó"
3`@ÅZ»g?קּ'›O¿ß¡D¾uñõ¿å`½§?õ¿áVÄ!Ølé¿ãÌ€ˆ¦'¿äŠšXz"AGNbll3FGL J1142.0+1546MG1 J114208+1547?ïÙè#)b?ƒløE­ê?‹É…÷5§F?ƒløE­é?ïÐÅC¥Àx?'׉0fï?w^-ø?'׉0fï?ïd´t<Rþ?'ún5î?"iqxu )?'ún5ð?îlÁ˜‹?—üÄû‰ò@?©3æ~GN.?—üÄû‰ò@4FGL J1143.1+6122?²ÀÄkËA@Jð² yLÀ:dIÄo0:À<"Ö"Üs3@±Fúæ:²?û͓fy±?Á9r½aÊË?ÐD¾ÂH@=À@ÍOª@xKôL!?ïñ­!5Ú­¿Ø´EíJ¿Ö˜"úUò¿×®«¤‰Ø¿è'I†[Ï4¿êÆ|†c[ðAGNbll3FGL J1143.0+6123GB6 J1143+6122?ïODOZû?˜æˆ°¦Ð?–—v ž?˜æˆ°¦Ð?ïôEyY×?mWÌaêlÉ?Wuñ
LP?mWÌaêlÄ?è•í6¸ìú?²
¶5o?ͨK%L?²
¶5o?ïÙ`S<Pp?Züä®ù?sOÖa×dz?Züä®ÿ4FGL J1144.9+1937¿ïÿÁ2ÔÞ@RAÓØZÀ:byz?a?À<Íùóv…@y¬'˜ï%?ÿÑ!%µ¿?º'ú E?~qB"ãÒ?Å6½+o"?û½'(z?ïL¾õsµ¿ã¥óD/Û¿ÒñO‡¿àÒýž%ðU¿ã›šu%¿ÏB7]xêAGNrdg3FGL J1145.1+19353C 264?ïò_WV0´?T–†É_YÈ?[AQSž˜?T–†É_YÀ?ïõsºYsr?f£+¿¼j…?U‹M?f£+¿¼j‡?ïÞyY\ž¢?v-GÐ]??pÃSQ°¯??v-GÐ]B?îÒuèĀ?
\->-@?¢Ø¯As·÷?
\->-?4FGL J1145.5-0340¿ïM{«½F@K«#c²WÀ;¯ä	)tnÀ<ßæ Zé[@ ½'³K?ùÌ(bÙ?àèä?°8?à'õ|ï>è?ýƒîÑíž?ûîi_jÖ?ë.2x"P¿ïÿò(¦è7?ïÿVW$ª¿Ü^äq¯¿ãü°TDz¿ïÿÀäa>AGNbllRBS 1029?ïèåt?d´>³TÔy?gçîí‹í?d´>³TÔ}?ïØô¾Fޞ?Œ#eb
qð?s… Ü±i?Œ#eb
qñ?ïOV¢ô÷q?P´ÙûÆ?–+¡aÒ?P´ÙûÃ?ì·¬æΙñ?ªéÓA(?ý?ºB˜É‹0m?ªéÓA(?ý4FGL J1145.5+4423?á_÷·#›@QèÑQ­À;z8«B9À<ª"á{°{@ÇRÏ۟ù@oÅÀi<?» ¤iT'¿À*Ðù'7}@äpùg@.°',ä?ïŠ[…~¿ærùпãÓõ €"Ž¿ç
:'£¿âŽ7€ŸÍ¿ðAGNfsrq3FGL J1145.8+4425B3 1143+446A?ïø—€Ö…é?NavSÔ?M¡ü¥èZÚ?NavSÊ?ïåG•š˜?'$ÉàÔՍ?jo¸jehD?'$ÉàÔՍ?ïCë?§V?•£e,éË?žw'˜&?•£e,éÎ?ï!Ðúʀþ?ŠC¦ؐ·?›Åযà?ŠC¦ؐ·4FGL J1145.6+5552¿ëÛP%€®@Msb¯È°À;¼±AV¥À=	l«$™@çX"Öĝ@=m;l½˜?Ìþ0­ï?Kèü}ÉjQ?}âkÅuëj@70Ûê÷Û?ïˆ?Õ%¿ß"ä"'ï[¿Ø|Õ¾Ž¿çÀùYó']¿ÊòëÅ`qÛ¿ïÿÿ&¦³AGNbcu87GB 114248.3+560915?ïô'%\öÈ?Zjœ>ãE?W±µFn=?Zjœ>ãL?ïü¡Óáu?c";gHV¡??Rñ`ôSü?c";gHV¡?ïh~—Ì?û"ÛTÝ÷?'ð?m|¡?û"ÛTÝú?ïö($c}4?DȺ~áÂ?S¯·9˜l?DȺ~á¦4FGL J1145.7+0453?â"'¿I4Ï@Og+©ÑöÀ:ìH£ÝÀ:À<t·×rB=@øW8ò@"{?;2?É\–#û¿³waì?çšr­™@ҘÛпÜބÛš¿é <€¹Îÿä†(¾e*ý¿íѾ¾í9?€ùu2˜?¿ïåﳁ¢,AGNfsrqPKS 1142+052?ïå‡vN±??«›/ç°¿?jx‰±NÀÉ?«›/ç°¿?ïøvY¨ï™?y'Õ«V~?N&™\Aœ²?y'Õ«V|?ïÍ_^^7?€
rˆ´N$?yPPÐ÷åR?€
rˆ´N)?ïü^äw
?9™½X°m??¥ÜGšª?9™½X°'4FGL J1145.7-6949¿ÙW ÏÂwÀ»?l&šÀ9èn"2QŒÀ;Ä]¨QÃA@c6æÆóð@S'ˆ?ŪD'?Ìûúâ´À'@é¨ÛUüŒ@\\¥t?î¶ãâ.V¿çÜ¢˜E܃¿è›¬>ÿ=¿î$Ä:Wã¿Û7ã¼R,¿ïñâ0`†AGNfsrqPKS 1143-696?ïð@¦ÇòÙ?h£w¹½0&?_~²pPg?h£w¹½0(?ïßÉGЀN?•¨Ûi?p\¿Ø°?•¨Ûi?í¡F<Ë?£)—OLãá?·"÷UΩ?£)—OLãã?ïoqÀ×B?a#Cû^Ã?'Þå§?a#Cû^Ã4FGL J1146.4-3327?ˊ@}v…z@;zãâ"À:æÄ©Ü¡À<€ëaŠR@26ï©@íàBËV«?Ïڿԗ?ÒmõJ‰;@;ç+y+?õÑÊWÒyà?ïõ/¢/k?´€îýÏ#>¿åÞ¾Ò8F˜¿äè)UJµ¿ïñp»Sþ…¿ïÿÿ)@k*AGNbcuPKS 1143-331?î´¢sYþ«?¥éÓJ™ë?¤µØÊ`l?¥éÓJ™ë?âwD5˜H?Ô*ñʤ|?Ûw"ÏoÚ?Ô*ñʤ|?ê{ô…"É?«»òYø'4?Æ/‰éì×?«»òYø'3?У'ãï.?±+Ó¬¿ï?ç®>±h?±+Ó¬¿ï4FGL J1146.6-2902¿íÄiÖÁç@?¹Áç–|¯À:ãòènÀ<Œ°"‡áá@_ʇù@<'Éä»?̟á²7Q?ь!f,/@부#§@†)ç0'?ä1£{š«?îúÁ'›ü¿ålÉVö†Ú¿è´Zåÿ¤¿á˜'Bdÿ¿ïûM³çùyAGNfsrqPKS 1143-287?í º¶#sh?°‰8³æê‡?²ú*NädÂ?°‰8³æê‡?ïšÂµ|<?œ_£('_p?‰OR üðã?œ_£('_o?ë¡Ìm¯?®‰óŠ·&ˆ?ÁxÎK"ñE?®‰óŠ·&ˆ?ì8‡óØ$?§I߂ìE?¾;Àa?Žá?§I߂ìE4FGL J1146.9+3958¿'ß«Î'Lz@QÝ÷'j@À7À¼O§@À;ŸÝkí@ådÉ-[@"ÚZT	m?"Mé=Ï?±/à~–š@ɝæ?@ZĨ»ö¿³ÊÅáv'$¿âáT¾É(þ¿æHmWoÈ¿å'pjÌ&µ¿ç½jΪó¿éÌò!+ûAGNfsrq3FGL J1146.8+3958S4 1144+40?ïޚÇ?°Åž¾"J?x¨²ó±û?°Åž¾"J?ïêYœØOÜ?€ডu¬?e¦c'°$=?€ডu¬?ïßy+$¾?qp¼§N?pCjm ¡?qp¼§H?ïýš[]?&ªà^ÎÔô?3+…#}?&ªà^ÎÕM4FGL J1147.0-3812?ïA®eá‡@6ô	å\ËÀ8v`' ×À;±d¾ÆyÌ@là{U`Û@G
=p£×? Î»do–;?«ð~ã"õ@.®@ð‹@½áÓo(W¿Å*F$§5¿àÙ§'æø¿ä‰¤úì/¿àõo]°à2¿è¬übf§¿àÍ7¡AGNbll3FGL J1147.0-3811PKS 1144-379?ïûá£ße??q¼ÅÚ?@yp'kÂ*??q¼Å±?ï÷û044?dj±'_ó?P	Ÿ—–þÇ?dj±'_ò?ïµÌd$|º?ƒ\͑3Ü?'ŒæöàÑI?ƒ\͑3Ü?ïòÝýG˜@?F±ÂR8úä?ZDpÏÇ?F±ÂR8úø4FGL J1147.2-2627¿íØ2Tx@A\1YÀ:
'@ßÄ À<T·«c@2—"@÷$œ—zÛ?¼]v}µ¸^?»´jÀ¾ ¸?ù]RV)Ž@ìéõýr²¿à'#€Õ¦¿ã{V'Ô?¿èÆB¤À>I¿å'EØQeM¿ëۙN?F¿ïíœtÜAGNbcuPMN J1147-2625?ïûžÉ5?> ['çä¯?A"Û+‡ä£?> ['çäm?ïýN]m¯·?NûðK©´?5''>Ì?NûðK©´©?ïàÈó[¤?r·R=½$?o7¤ú[…?r·R=½*?ïû8w"h²?3µ×/ÕBÒ?C!®]:	?3µ×/ÕB‡4FGL J1147.4-6758¿·þu$ØP
ÀhaýKÚÀ:I:MÙ§§À;Ë
ù½Ç@_‹p¶÷M@§ø-ýi?Ì@x@-˜?ٿώH,¿@žÈ~‰rÛ@uœ9\¿Ùçwþ"E¿ãRôÏJU¿åD(Müã¿ê­x:¤A¿ïþûž‰s¿ãlqãr*ÀAGNfsrqPKS 1145-676?ÏFŒì‰Ö?Åq2ãC¢€?è.\ÄݸÊ?Åq2ãC¢€?ډÙÈÏH&?Ó˜îÄ	Ö?⻘[í?Ó˜îÄ	Ö?ÊÅÍ]1Î?°±'¨ýÂõ?éNŒ¨³¿?°±'¨ýÂõ?Ñ¿`é°»?°aù=Úè?ç {ϋ'¤?°aù=Úç4FGL J1147.8-0724?ï'L£ÎÈÇ@JßeUÅÀ9yæ'æÀ<TTëêŸ@d"ZD[@¯¸õs~?±òù²3†?Åä=;IØ@Ø\$ħ@~¹*³?ïÚua«ì'¿Ùº·Á¢Í¿çêßÂrÖ·¿ç_XŠÛµ¿æ…Lp¿ïõæÁÀ7AGNfsrq3FGL J1147.8-0725PKS 1145-071?ïó‡Rî?`¯VÙ{'?Xñ[ËÂ&¸?`¯VÙ{•?ï÷ÿä×ÿ"?i½÷΂>3?P6Pٖ?i½÷΂>1?î‹éóæj?˜ËHèXç[?§An°Á™O?˜ËHèXçX?ïðÏ{©??Jú¡Ýq?_Ìa­€Ë?Jú¡Ýq'4FGL J1148.5+2629¿Á0øùËϸ@RýàŠï²«À:–°ä+ŽÀ<oÅµW@£I.G;(@§±9ÉOj?ɞ¥2?¼HÛæñN?îõù`½°@¹î£·*¿ÛBž54À¿æ;T»,¿ëSà4éí¿èvk—'ÏR¿ïÿ³©æ÷¿ïÿè+ÍäAGNfsrqTXS 1145+268?ïÿ/±œD·?°ŒÞ±ª`?	Ìwi>è?°ŒÞ±ª:?ïüª¦Ñø?U^«<¯S?:ªÏ)p?D?U^«<¯\?ïàž^L:?o(E#?oa¡³Åø¨?o(E?ïôztÖ¯¡?H³}†©?WR ¾ð?H³}†©4FGL J1148.6+1841?ؕRÔF*%@RQ'U°5½À:œ2ƒ
À<'HÌ!¬"@ÚÏE"@7›x¦?Äuƒ9ÛÃá?§e"ÏãÙ?ãO؅g³n@Æð)s@ê?ìô´!Û¿ê&$V÷]š¿ãÃQùÇכ¿×$:ýöe¿é Ÿ>À¿ï÷,ÊxAGNbllTXS 1146+189?ïùI§"4ð?E
ªµ¶"?JÙa¯,@û?E
ªµ¶¸?ïü)}Ö±à?T(RÇ!Ì?>´Jq?T(RÇ!Á?ïÜýÚ{X?wŽ¸†-²Ë?qøÂT?wŽ¸†-²Ò?ïéÁå-{÷?RÇ#ìEòR?f>҄	}?RÇ#ìEòQ4FGL J1149.0+5924?ډY?õ}˜@Kû`¿]xÀ:¼¬'\fÀ<—ˆü"cõ@S*¡iFÁ?ýØPXÝç§?ÑC¢A2û*?ÍwV	L?ö<py@œúåcǿᲈˆ˜À¿éu0™$ÿ"¿Ô£"ŸXö¿à—¢H"Ä¿ã…WWÕ©ë¿ðAGNrdgNGC 3894?ïóÎ_ËB?Xþ¦ÀQÇÑ?XcAði|È?Xþ¦ÀQÇÃ?ïûü\|?W¿"uΔ?AûäŽ?W¿"uΞ?ïaë̾?'Q*Šd?"ßb†|H<?'Q*Šc?ï"❬Òø?uwn7DU?ŽÇX"ËB?uwn7DU4FGL J1149.1+2819¿ïµû >!@S
†½ôµÀ;5º>TÏeÀ<¹šTbX@îÎxžwO?ú:73rô?ە̅0b?ЮrĘ Ë?ã ýy¼…@œVUi?첁Çë¼|¿í–ðÝMM'¿Ü¶¡gP¿Òòœ"%¿ä°Ëæ¿ïýYÝl[AGNbcu3FGL J1149.1+28157C 1146+2841?ïþHµŠC.?&ûü(rK_?+t§[Ís?&ûü(rK·?ïüúxæ´Â?P×ZQÅW?8,8ÊYó!?P×ZQÅVô?ïÇk8i+
?~ÿK'ìó?|JcËj{l?~ÿK'ìò?ïõ[xR$O?Cÿ1u`?UI[·b?Cÿ1u`+4FGL J1149.2+6246¿í'"÷¾D@Juü–þµÀ;C`dÄ¥·À<➽ÅÈÍ@î]ìn@åRº·÷S?Ä(2y$?¿¬'Ó|"P/?啬¿ç<?üUŽ¿öЁ¿âVà±09¿á?-!¡:x¿áOÝO³¿ããY '¬m¿áVó+Ü'¿ïÿÿ)@k*AGNbllNVSS J114926+624333?ïôKGàû3?T	«ðÇu?Wip>	›3?T	«ðÇp?ïé-/Q¹?€=Œì'Xþ?fÒЮFõö?€=Œì'Xý?ïˆéÚ^å?"ù0½ðÁ¯?Åº‰hF´?"ù0½ðÁª?ƒ³‰?| ¶ÿMXµ?Õ_¼…?| ¶ÿMXº4FGL J1149.4+2441?ì	Êó/£J@R÷l7`¿]À:îY_æÌÀ<
ª}íl@ ÉêWÍ|?ýz¬(©l?ÎՑ—l™?Äk«õ'½?ùƒX´Ï?ú^/5L¾¿ê{`"¾ŽF¿èç6žË2¿àÖ|x÷c¿Ø]]¾¢¸¿äå}ºŠ¿Ò^(_ÀñAGNbll3FGL J1149.5+2443RX J1149.5+2439?ïúS‰=]Î?Eì"s©O?F±Û
ˆÉ‰?Eì"s©3?ïŠ8Í9·Ö?«‰ñÏ
$‰?q̱'
W?«‰ñÏ
$Š?ïڎÒøâ?tä¦)¨?r¸–ƒó/?tä¦)¦?í}±{tw? {!B'Ì?´Êt$\H? {!B'Í4FGL J1149.5-4029?Ê7=ïÈoÔ@4Þf˜»MIÀ:(3û°À<;šß÷.@-' %ú»@lŠÅÁ@?¼†êªÙ2?ÀbHIšÓ«@ÑÄ2ÊW¨@
®"ѶkŒ?í€ÿ90£6¿ÅG³Gë|¿åÓ áŒwr¿ç'
~ß0¿â9ã¡$¨V¿ïÿþó…õAGNbcuPMN J1149-4029?ïæ޺ɧ]?ksá^~?i!E6X¢J?ksá^y?ïönšJ?jÔêj+$¦?Sé#àËm{?jÔêj+$ª?ïy®a8@?Œ9U|®?Ê3ܘø,?Œ9U|±?ï¨fÕ$?lB´!˜>Ò?…ÿ¦J¶û?lB´!˜>Ô4FGL J1150.4+2418?ÔnXe
mÉ@Rþ€sWæqÀ8Ý^žšÀ;ÿ…ÄÐ	@
;ƒcÍ/@Š82vtÑ?¤ð?éØ?­‹ÊNe!@Ñ™Sù|@
H¿ "_ž?éT¯àÄ¿à
RÎÙí¿äF¼x{¿áº(»
,ª¿æ¤Ùžlg1¿ì~õ†÷AGNbll3FGL J1150.3+2417OM 280?ïõ$`'m-?Me,»¥?U·>Ý%¦?Me,»¢?ïÂx+-ÂB?"Xê®?~Ãêiމ?"Xê­?ïÃ3ýaO§?%çëx;?~fOX,"?%çëx:?í֓΅ïm?šËæ÷ÂB?±Ka‹Ð"–?šËæ÷ÂA4FGL J1150.6+4154¿Û'¢ïHº@Q«øʁ˜òÀ8²¶d«{CÀ;š‹'!­@"³<Î?ùæ)_tڝ?¨î´Âٝ¯?º?©ƒ	@ãá!îgQ@§‰§´¿Â¢£C â¿ÓvÍ;Ý{Ç¿Ö+P%\Zõ¿ÔjzýÍÙ¿Ü-þ`BµÝ¿ä&œˆŒAGNbll3FGL J1150.5+4155RBS 1040?ïô¹vf´Š?Y¤íÅà	e?V2–éú?Y¤íÅà	n?ïí2W~?|:Ä$üÜ?bîͨíä?|:Ä$üÜ?ïÉCLªKR?ƒÙ'&j?{^YªÚV¬?ƒÙ'&m?ïŸzÆÄêç?s_}Óä?ˆ!NNÅEâ?s_}Óã4FGL J1150.6-4823¿ì¦•å=ãƒ@*…ê̒jÀ:,Ù=—ÀÀ<Uäßq@ZT4_®@ÕM¾Ñb?ėܕ—¬Z?铙¥X½@V́Mrz@uOVTux?ïýý'¶œ¿ÅŽ"½"u˜¿è6u¨"ÉY¿ïÿ°NçÄ ¿Öÿïcû}?ïôlj£'AGNbcu3FGL J1150.7-4816PKS 1149-480?Ç$|°k=m?Ì
´ˆXk?ê6àÓå0¥?Ì
´ˆXk?ÿNwÏ?³«Þ³‹>Ô?ïŒAˆ?³«Þ³‹>Ó?Ö¨Ägýjm?¾Hµôv'?䫝ÌJÉ?¾Hµôv'?£Ä,"?¢?u×ÄÒ?îÿž½7'?¢?u×ÄÒ4FGL J1151.3+0957¿ïcÔ*Íë@Pï‡~äâmÀ9î{Üð0À<^RèÛ M@Xx]Öu@9^á6ç?³ê©ó¿ÇuçY?Ùæg¨…ŧ?ûáHÒ©¿å")uš¿â¢âƒw¿ç9iãÉh"¿ß?üoQÇs¿éa[?êx¿âðŸdß©AGNbcu3FGL J1151.5+0957NVSS J115117+095826?ïcïná¤È?^£e:Îâ?"'#Ëfæ?^£e:Îã?ïÇP㌨d?'°‡ŒŠ"?|WŽ9«ÎM?'°‡ŒŠ"?îÆÄÐ^'a?–U"ä»/Ô?£"²úÙù?–U"ä»/Ï?îoH»²xè?›¤&aIÜ?©tDØqŒ?›¤&aIÜ4FGL J1151.5-1347?Õ;bFµÝw@GIÿ¼ä!À:+oðSÀ<L•¿ðEx@Fs´N?þ¿4"…ƒb?·ŒÍ|²?°s¿jc¡?ø õäKj@´~wTJZ¿åVÛó[¿Ÿ'gB¦»
¿á×&ø'Mu¿Û{–yS¨õ¿Üë±~è"R¿àþp·'©AGNbll3FGL J1151.4-1346PMN J1151-1347?ïúÒ	œÚ?D€ä!´¿?D·‹ÙŒ™?D€ä!´°?ïûÒ&Ü0ã?W@¬öHp?@·d<xï?W@¬öHb?ïôÓUt>?`XB¼õ<¨?VYUƒÝ¸?`XB¼õ<¥?ïÚ
R'ã€?\'¹+öTk?rúÖ¶Ž@¦?\'¹+öTZ4FGL J1151.5+5859?͘¡®¾@L>-b8Ú<À9¢àJXçÀ<U¡E@Ý\u éZ?ûY
Ð>?³ ôpTÒ?·9@þÍÐÙ@ÅÈFUNç@OKí"C?ä
¢»Jî¿ßBÌ-jœV¿ÕpàÝûÉ:¿Ý8 z´Q+¿ÙùÄ6%¿ã¸ãÁ…ñÇAGNbll3FGL J1151.4+5858TXS 1148+592?ïëNÙl?c­µ¢JèÍ?d±âñ&"&?c­µ¢JèÌ?ïï}Q²p?sœ¿6µ?`'®Méþ?sœ¿6³?ï¥B '¸?‰GN#Z_?†¯wöù?‰GN#Z[?îÓ%ÈÍ(ý?"ʬ¡>Õ}?¢Í£s-p#?"ʬ¡>Õz4FGL J1151.6-2115¿Ý:Qà¯@CÀ¹w…r›À:üõÊò×ùÀ<–þï^È@ ~Þ¿¤ó?üáX"Ì?ÌëÔWÜ?»k/ùÂÏ?ñµ¡7Ì¿?ÿ8¤aHÅ¿ïênió9?ïò`ŠÚ9¿àh"¾é_U¿Ñ²ñCú€º¿ä
d½™Óü¿ØhÒý='íAGNbcuNVSS J115140-211345?ïþP6}?,YДO~F?*÷ìž8?,YДO}ã?ïø,Rànã?b0`])½?ON´~Dx?b0`])¹?ïð~œa´4?bcº:<ã6?_Ç<—™X?bcº:<ã:?ïNuü?€¾×Ð}Ë,?–/Þýñ@[?€¾×Ð}Ë-4FGL J1152.1+2837¿Ô%/%P¢i@S40@9«óÀ;aga8)<À<ć0
‰Ç@!?Žµâ¥?ýÀ(Ê#¥!?ʑ8wß`?W]άÖ?ÁåŠ2ôI@ù
¿cí¿íIn¾¤•÷?됫´NPÆ¿áѲ_c<æ¿áqùAŸÝ€¿¸½=ã^¿ß$ù9{øAGNbllGB6 J1152+2837?ïû¸29"?B,0ø«ë?A‰7°R?B,0ø«ê?ïý'´O?M[Í}™?4ÇÊ]'%?M[Í}¾?ïçùöS‡4?j"œ:	#?h	¬xÍu?j"œ:	Žö?ïî¥þ1Øa?UªñÑ
…?aZÎ'Ÿ$?UªñÑ
‡4FGL J1152.3-0839¿ë'Ò`Sà@I¸ÿ!³®ïÀ91÷ÃœcÀ<¨Ü,¼@ïapˆSK@è#½tj?¯
^\N,?µIȔ.@|Úa
@å،s–?»kÂíC¿å;*®)s—¿åÁ »¿å󾩛¿ê"œý|B¿és$ºÊlAGNfsrq3FGL J1152.3-0841PKS B1149-084?ïøíu!?BYâá=&3?LJ+{籖?BYâá=&;?ïú4hf<Þ?]jï|KÙu?G.^gŒ¼?]jï|KÙx?ï´ûª/!?{%p?yöñ?~¥'*èo¥?{%p?yöñ?ïü ‰õ?.1*G/¬§??*û°Yû?.1*G/¬Ü4FGL J1152.8+3308¿ÈedÛa@RÿÀ6âëÀ:œÞÀXÀ<}׺f˜»@§õýȘ@´Å¿'Q§?¾]b wóñ¿½TÂá!Ô¢?þÍðÁ@Ÿ¶2+¡D¿Ô¦"Sß{%¿ìwÅü-ã¿ëÕ9¸ˆr*¿Ò¥ñ7"+¿é(ýOL?³E'Q}¡AGNfsrqB2 1150+33A?ïü'"ø?CrAƒ\ѳ??[oØ9µ?CrAƒ\ÑÂ?ïñjv}Ž?'€Օ™?]ß+áY?'€Օ™?þpºõ?…¸«ÖˆGI?‰ŸÀcÑBÅ?…¸«ÖˆGM?ï߯!Ì|?hqã‡Ém£?p(oÁó?hqã‡Ém°4FGL J1153.0+8056?ïèfu>Àº@Aï îؐÀ:+jК¸À<_ÙSÃÌs@}à}Ù @Zt:dÜ?·hfEÚ*¿¯Œç.¢Õ­?ò×z:XÁb@ꗶ?—›?íº¾?©c¿äÌ°èj¸¿ê8±ø50¿æ¸/â縿ì̼¦äÛ·¿ïÿŸzFAGNfsrqS5 1150+81?ïþêÐ寃?$瘓Û*?!Rñ¥Í>?$瘓Û*Q?ïý–ÇÖ?MƒQlæ?3ƒIÁL½?MƒQlæ?ïØ]³Ë%Š?wÙTŸrjª?sÑ&m;"?wÙTŸrjœ?ïüeZ¢m?-ø4i	Xs?<Õ/ìš6?-ø4i	X—4FGL J1153.3-1104¿Ø8‹}£ó@H¤eƒèWmÀ9ð4îõÁÀ<6¶³…Óê@clùþ^?@0>Œ,Ê?·c´Û>˜?²ù¤)ëa?øopJ붝@8ßwŸHÛ¿Ålê¹ò«¿âõ}ðñš¿æt«"­ÿØ¿âvO¿êñxô¿Ù8ÊKéžAGNbcuPKS B1150-108?ïùÙÊÜ?Aýj°-êƒ?K ˜Ôù'?Aýj°-ê?ïüä÷ûäÜ?P°'Ì'v?8Ø@ Ùõ?P°'Ì'{?ïßT…¬¢1?s=ëÜâ~?pU½)®ç?s=ëÜâx?ïÿ]?ÈA?^T÷Hr ?X÷Î[?^T÷HrÍ4FGL J1153.4+4931?à0£ªÍP@P?W}•WÀ8Þê'ò#À<AÌN!Ì@˜ üö@ŽŠ#Û?¢Ã^äçˬ?£ãñ¬€&+?þäԕîê.@Hm²(‡¿Öыؾ¿äÔú˜¸¿å‹MpÌö¿ãs>í¿í=HËJ썿ß9Ü>YØAGNFSRQ3FGL J1153.4+49324C +49.22?ïú¿è$ôî?@ªµ¹6ò?E_l,Mû?@ªµ¹6Õ?ïûÜoÙÀ?]7èJÌ?@ŽCä™™?]7èJÌ?ïÕp
»´?x€÷u¾]à?uGú¢%ôÐ?x€÷u¾]Ý?ïÿ÷'TÅ>Ñíàâ9ò>Ñó±Vv
'>Ñíàâ:¡4FGL J1153.6-2553¿Üƒ+­QÛ@A–ÃÉîËûÀ:…wqP¥4À<mgZ',–@ BP¾ßNZ?ü5 *­R´?Ãõ]$H^¾?ÆÙHƘUL@1æaÉH´@Z9è4¿ïñ¸ðiŠ?ïE®*JVe?®@ê</—Y¿ß)¦W>
¿áÊ°]*}'¿ãž™]´'AGNbcu3FGL J1153.7-2555NVSS J115338-255412?ïú0¹ëš?Dø‡úR›Ú?G=SњÕ?Dø‡úR›æ?ïúBæ>vÛ?`­
ÛB¦?Fôg$8?`­
ÛB§?ïÅ"m6Í¢?{["ôâ£?}nÉd™.Û?{["ôâ ?ï©OÉå>?pÔgwS>?…¿¬
†°ˆ?pÔgwSA4FGL J1153.7+3822¿ï©Ô+¦à@R`{_ïJÀ;i°Œû%¦À<ç¥'lU"@ ¨RÑ^,?þ­é—Þ®w?É´—L?yœèƒŒ'ô?µm‰_(žI@vJ_É¿ï7óâ:rB¿ÊRŒ)nŽS¿Ð¢0aFÁÛ¿è'Ø¥H#…?Ã^jÄoF¿áPå*'¤AGNbllB3 1151+386?ïûñtT6?=BoÚº?@:/†¯%1?=BoÚj?ïý¼¢"þ™?J$oùŒ ƒ?2ëX8m?J$oùŒ œ?ïÃaE\¼Í?}£'W—]?~O]Q¡š?}£'W—Z?ïúéç©¡Ó?=>«)¿O?DXaYx¶"?=>«)¿G4FGL J1154.0-0010¿ìzìÅñ]/@M³þCg]ÝÀ:ÄÜ=ƒÀ<:贉ßè@ ¡Øñd?û¨À˜áãµ?¾(²?œ'à?®1´%Ÿ!?óêIš}Å(@ÉÌJØÁ?ï÷±j8X?¥^w.µ ¿ã?@óVµ¿ÔEO_¹£û¿ÉÁJ£g†¿æ-h¹&ý›AGNbll3FGL J1154.2-00101RXS J115404.9-001008?ïý]ÕA
"?1½˜*·"?5U÷"h?1½˜*·?ïüŽcBoj?QWó cÞ?;Œå섲õ?QWó cá?ïî}VÆ?m6ÍZLã?a'÷í©9u?m6ÍZLÙ?ïå{ºç,—?Xôé,Œ9?j"EÓi‹?Xôé,Œ@4FGL J1154.0+4037¿îžµ
F @RؤTÞÀ:KO7u¸À<Kžd¶@ŽeÖÉzÞ@¡·D¥?»©¥Ö=ä½?žçÚø½7?âÙV}»Â@
€#½Ÿ]S?ï¹OýnUH¿¨³oX¨bµ¿áŒÈ›䟿á4Âkðê¿å:c©Ä\¿ÔdfÜØÞ~AGNfsrq3FGL J1153.4+4033B3 1151+408?ïûú`A?8—
Ýá|þ?@–~ûã?8—
Ýá|ß?ïüý±™×9?TpõEDéÍ?8s1F;Ê?TpõEDéÏ?ïïŒ×¹Ž¿?f§r˜ÁM?`s(FqAy?f§r˜ÁM?ïì-"i?R_v‡Oä?cèÒkì˜+?R_v‡Oá4FGL J1154.0+6018¿î[" ¥{ä@K³û?¦ÞüÀ:Ý]=ȸÀ<FDw(UŠ@ý¤)j‡ˆ@j$aY?¸ÅxqÖ²?ÎÐd¾›‡@AÀ6@ÓÖ;‹qc?ÙêY¥Ã£¿âRƒÅò½ø¿é³ß¿ëÔ9~§¿ïþ{ ۑ?ïêӝ÷LRAGNfsrq3FGL J1154.3+6023RX J1154.0+6022?ïÕþ¼!/?y¸m
øÌ?u¡ïhw2?y¸m
øÌ?ïñ
ê Ç'?wøSQŠÑ?]ä+¾q²?wøSQŠÑ?ìçT_Èl?£KÃ¥‰'É?¸Ç]¼ž?£KÃ¥‰'Ê?תּˤ?v¥³ù£?"»M8—S?v¥³ù£4FGL J1154.1-3243?ïeA¯åžX@<Ÿ¡<%J<À9Tm'LžÀ;ñ´#ìn@"XWÚÝ\?þðCå2`?®wE0áŸB?¾ÁÀ	@t\!iT@
¨!"Šé?ð¿ÜÉ/^giq¿áª¿†¾ ¿ÙœF‡£Íпç¨S;wG¿í™šùdAGNbll3FGL J1154.0-3243PKS 1151-324?ïáå‹]§Ò?¨WçøÐ=t?nt¢X.P?¨WçøÐ=t?ïàB%¹?‰eg-@-a?oþù½ÚGw?‰eg-@-`?ïäO%ô?–-k
^ŸY?žnVA‰?–-k
^ŸY?îù# ·îf?"×Qxù? mÍô°?"×Qxù4FGL J1155.5-3418?â»>ÛÌN.@;%ðÃL‹À:=Áz‰3À<O»S'ÅA@ ³‹WŒƒÜ?ûъŸb0?¿ 8Åxr?³yx€´	K?öœÜ_@Ÿ1czN?ïþ»ýq°G¿ç$O€íl¿Ó¼GÃe¿Ð\¢õ¸Ô¿äbÐzw¿·Bï=åé©AGNbll3FGL J1155.4-3417NVSS J115520-341718?ïÿ~TFü?aÞ\º²î?5lW œþ?aÞ\º³Ê?ïýíót˜Ò?Dê\þA?0d[9h;?Dê\þ@?ïù"Þlö§?\¹6¿½«Ý?I¬†L%e?\¹6¿½«Á?ïÖç2Ø?^'ÔAt«ý?tŒ1fÀj?^'ÔAt¬4FGL J1155.6-6547¿×8è)Ÿ_ÀR¶ä-;¢À9Ö%Ü2›^À;;u –
@Åv¼ƒ)@ê໗?ΛraÇEN?Õ« ,ZÒ@	WQ:…7?ôxƒ<
d?ïç)€=Ó¿áD7%?U¿é¤óÕORN¿ë¸ðvö£¿ïýwקò?˜cï=ºöŒAGNbcuWISEA J115414.97-654215.0?çÓó±<Æ?Í¡jµîœî?ÐYø†v?Í¡jµîœî?ÝG–ì\ì?Ö¿ùÕý\?á\4‰¸QŠ?Ö¿ùÕý]?Ý4†,«ÎÙ?¹;Ì´"³{?áe¼éª"?¹;Ì´"³{?šìáž~??"ø±®ûç?ï(˜óÄ?"ø±®ûè4FGL J1155.8+6137¿äbÂ0mOõ@K!ýÞ½À;˜Mà]£À=™0¾
í@!
øæ0K!?úèÎör¸"?жÙÛÓûÀ?ŵ¡bê"?ö¢XOLnn@)¬'½¨?í#·•-#O¿æÈóĈZ­¿æ×z:XÁb?»òð"wÍ¿ÝÉ/‰Z‡5¿ä,\\×qAGNbll3FGL J1155.9+6136SDSS J115548.40+613553.8?ïøí–&R?LûbÓÇ?O¬I§fº ?LûbÓÏ?ïú6Óȗ?n+V/Ú2?G'Ì°Ý ?n+V/Ú5?ïÊ[iÜó?}v_IáÜA?zÒuˆ?}v_IáÜ<?ïʸ»cr·?h͸šå÷ª?z£¢NF¥B?h͸šå÷¦4FGL J1156.6+0640¿âp;m&bö@PpmH÷QÀ;eEñ{ؾÀ<¾Lj;Ýý@HãHº.@q<î×í?Ø
PJ›.Å?Ó5ÂÅ+?õã]gº#}@
Ì3j¾9¿ïõð¢i÷À?ïö$´ë.¸¿Ñ·	ìèÌ¿å
ö~!)¿ïñÖ¤¿î×oZµAGNbcuTXS 1154+069?ïù"œ¨å?S%#ônÓ?Kwñ\n‡?S%#ôn×?ïû
Ú»¢?Y+Lm°?Cȕwîý?Y+Lm¨?î(vÆ܀?šA,Ñ-ë?®-x"'8
?šA,Ñ-ë?ïÞ]¨TŽt?aXªè–¡_?pÑ+Õ¸Æ)?aXªè–¡[4FGL J1156.6-2248¿äˆ¸m@C+8`™ËÀ:mAaÊsÀ<_†z%@ð\ñržƒ?ÿ"òXwZ?ÜW¹û8ñ?ÄǏ¡F@"à¹(«@¹
¨4<¿ïÜl²°Â?ïÞÁÉ'¿Þ¢T~1‰:¿á[¹.׿ۢÉä:&¿èG犾4"AGNbll3FGL J1156.7-2250NVSS J115633-225004?ïÇ`±‡¡?òó'h¸?|O§</p?òó'h¸?ï÷‰ÿ†S??gF¾ ÕÙ«?PìóYƒ'?gF¾ ÕÙ¬?ï'éa5T?‡Öäð|‡™?‹E§¸ò«/?‡Öäð|‡˜?îÆFt
HÃ?ŽÝøŠå–?£›˜¿[sÇ?ŽÝøŠå•4FGL J1158.5+4824?é蕪Äw@P—BÃÉîÌÀ:3(¦É-À<…bÎ+qž@iXûÓö@g6:N°g?¸bÓ3ïÕ? ®Ý½NÄM?âÆ8Éu)x@ O¼€ÏH?Ý	ß<fÏ¿äŠLŠN¿åµ‡k™¬¿çµ½A›"¿èWõ¹€¿Ýõy(àÉÚAGNfsrqGB1 1155+486?ïýˆémü?-KN!4	D?3¸´ŒK?-KN!4	‹?ïýíºFÓ?RÁEá€Î)?7è'-ÉoX?RÁEá€Î#?ïê?4˜Ý?i1ĝj¯õ?eÀËøg"A?i1ĝj¯é?ïÿ:O'£?ƒß½½2?¶k¡É?ƒß½¾l4FGL J1158.9+0818¿ïê=9É\•@PܵÜÆ?À;ˆCaÀ<§óv"Á›@ 6°Ë9yÉ?ý[ÛÈé~?Ê@åxjIö?¶ºùw]?î<G
ۊÖ?ÿj?›Ü??ï‰þ›üË¿íP_ÿD^¿ÃEyÇAGž¿ÚÚ¨!ò™¿ä‹ÂÁ[)œ¿Õl—£TYAGNbcu3FGL J1158.9+0818RX J1158.8+0819?ïþqw£C­?%"¢TÃ#?(è…ËÅ5±?%"¢Tà ?ïúeØ8*x?]>ÝUì-"?FhŸV!?]>ÝUì-"?ïóm¨Òm??cþšt£'?Y$®[%ë?cþšt£|?ï^^û.ãÜ?~)ós^È?"4 š#"z?~)ós^Æ4FGL J1159.0+0939?ӓ|Dxã@Q&8ÅCÀ9¼b †ˆEÀ<H}'ÒÕû@B™³šÌ @¥?|í'h?³Î#Žû[?°ý<aNÏ?ü«ÓXI@7}	Àóü¿àD'❪?ÓÚL|°TÇ¿ãU38;°°¿Þs]$žDú¿åÄz¿ç=W^‹¦'AGNbll3FGL J1158.8+0941GB6 J1158+0937?ïûb®î`?B§Š\‹R?C'uDF†‹?B§Š\‹{?ïý7ø¾–?LQÓ×õn?3~@:Nï?LQÓ×õr?ïÔõ€…X?|TÎaz‹?u…?½@T6?|TÎaz…?ïñi8^C?Iÿù†¼ºÈ?]-ÁCz?Iÿù†¼ºÛ4FGL J1159.2-2227¿®Ì,qj@CjmŒ?À9/v>J¾jÀ;ÃQvëè@–Ÿ¤J¢'@Þ¥rðR?¶fŽ_0½?ÂKD÷Ö»¹@€	ö#l@3M™Þ?׀ÒbãÏô¿ã¶"v¿æ–îÄnYz¿åX³ UöW¿ênjЛ¿ïÿ~€8Ÿ"AGNbcu3FGL J1159.3-2226PKS 1156-221?ïÛxYû
?p8©—?rCÓuz"?p8©™?ïûâICÑ?S )uÀÑ?@wêÚð¯?S )uÀà?ï>K?—x?#;ªÿÂ?˜6˜
q
?#;ªÿÅ?ïô2Ñyõ?FÉ×3ˆ?Wõš]¾?FÉ×3ˆ4FGL J1159.3-2142¿Ñi© V@CÈú?̞ªÀ8ÞqÍ¢µ¢À;¡"ØaV@¸‹Í(<@çüÓû•?ªD?è<.?À·—FBÐ@á¼ýKð™@3®~Øù¿ÛTbWä¿âûîç´°¿å` ‰wãf¿ç9Â,_Ú¿éá1ޟ](¿ïþžÖð<>AGNfsrq3FGL J1159.2-2141PMN J1159-2142?ïñ[åÕ><?Y¼À{ÃëN?]H4Uƒ†
?Y¼À{Ãë@?ïì?z.'?u­1™db?cÀ…ëÑn§?u­1™db?ïb°ôuV?'†[es?"©áqU<å?'†[eq?ï_Š~y?"b[¢çî?¼ð0¼?"b[¢çï4FGL J1159.5+2914¿³ qØî%@S˜	¿œb¢À6Ù¾´Ü?À;tR¸3¹@
ÍËzgO@ӎ¢Å'F?‰ÕQðQ{?¯óæÖ¹5@"2~À¨@!æƒ.Äd¿Á8'Ù÷¿ß#½ßÉÿ"¿ã¤Û·K[H¿âóύd¿æT+
oÆ¿ç¶é¡éÜAGNfsrq3FGL J1159.5+2914Ton 599?ïàôb÷?¥Ìûhi?o~ëÇ?¥Ìûhi?ïã^¨;Ź?ƒÀž=©?l¡WÄ:F¾?ƒÀž=ª?ïÙĝ[vT?w¹Ïÿ~;ì?s±RDÕÈ?w¹Ïÿ~;ï?ïÿ9Cö»M?€fg?ׁ(–_{?€f¸4FGL J1159.5-0723¿³
m(™Q3@J¢qÿ÷œ"À:&Nɑ®êÀ<M@± ÷@¬úv~6'?üæ/Äé©|?ÆÉGÝc?ÅڿԖÆ@ÖÓßÅp@ò´/œû¤¿ïÿ틉5ž?ïüî×컿Þ7Ó@"TŽ¿ØoE2980¿ÚMâa®z¿íŒ_¿ƒ8.AGNbll3FGL J1159.6-0723PMN J1159-0723?ïúŸÜÎľ?AþxÖ&0?E€ŒÄí?AþxÖ&*?ïù!úöaä?_î 0ç ú?Kx&xpƒ?_î 0ç¡?ï«OÉï+ö?"lhð¬?…,
"5¶?"lhð¦?ïzìa®ùÃ?yæ"Õ"‡?¢sÊ Ç–?yæ"Õ"‡4FGL J1200.2+0201¿ÄDkféF@O–#ûÀ:(*ùÀ<nΠâc7@Ý0õkL@Cx$Õ?½Æ'ÊBXë?½Àdß}©y@jä°a @\wûT¿âõõ»Ÿí¿Ý­† J¿á€>´pµu¿ÛYÄAê¿åSP¦^N¿æd¶}Õî´AGNbcu3FGL J1200.4+020287GB 115739.6+021927?ïüś*bj?W¢~é"b\?9Ó&¬ì¬6?W¢~é"bj?ïüV¥>,?Sí§Žýa?;•JÖ¤?Sí§Žýb?ïðBÍxd^?i€mΈ\?_ze7B¾?i€mΈ`?ïõ¡Wqeb?@îžMUÃð?T½Q585?@îžMUÃß4FGL J1200.6+1229¿êÆmâgL@QÉD=F²lÀ:^4Òo£ýÀ<v†oj@÷÷ÔãF·@"Í–&?Àíá\Ÿ?¼¥Ú5@)?ùý ª/@
|÷ÔÃ?í•÷ƒY¼4¿äy'"¿å79ó@ÔÜ¿åÒÑɋпå\ÏAS¿ïÿLa¢—AGNbll3FGL J1200.8+1228GB6 J1200+1230?ïûíÚÆ/H?A7¿Õ¹¹?@H"çBßç?A7¿Õ¹Ä?ïúÕtSý?XF3=	7?D«Î.°	;?XF3=	:?ïê Ñûã?hw¢gë+S?eðß.Ô?hw¢gë+^?ïÇêò¿¡?i#¼Ïr?|yŠ† /û?i#¼Ïw4FGL J1200.7+2008¿ê¸ò(ì)@Siì,äeÀ:´Ç‰¤À<l´ˆ2i	@Yï`÷'@âÿœ,ñÑ?·ƒÀë?©Ýì@Õæ?ð ó*.§³@	å·Îí?Ên¸ÅXå¿å­U¾xv3¿ç'ù¾ÈR?¿âÛ._ƒô¿ïþ|§ñK1?ïÚ¡–'õAGNbcu3FGL J1200.9+2010TXS 1158+204?ï÷°;¡?QøP1	ž?PŸÁñˆ½&?QøP1	ž?ïüjÞ]f?S¶7(‡y?<©%Ó­?S¶7(‡y?ïÚ¬ª"??v¸ƒKýçR?r©ªö¶`(?v¸ƒKýçR?ïåXø¸Ë}?`';eî·?j§G4"J?`';eî¸4FGL J1200.8-1429¿ã —±`5S@GMØ@žUÁÀ:é'm{.À<vRNmS@ VÀ"Ûë?þöíï/Î?Ë«¾à%??¸·²3nlo?ìç¬sßÌ@CIËûìu?Àw¿ïçågÎE?îYœô—ìñ¿äˆ-@U¿¿×vÝâžÆ)¿à¹Ö?è"iAGNbcu3FGL J1200.9-1432NVSS J120055-143040?ïþbѤëà?%?t呷l?)Òå±Aö{?%?t呷
?ïü_Y局?`±ðÁX?=0ÒtÀ?`±ðÁY?ïñ•çáÔ.?hL}ô2
Ý?\Ô0<W¥l?hL}ô2
×?ïîÓ·¬d?T"ÛH½â›?aì,HS›è?T"ÛH½âª4FGL J1201.1-0332¿ïwO£é
@L'"¦óõÀ;Ô/—@À<nê™fn@Hÿ¥è?þ­[î=_Ý?̇'™£?ÆÂáfŒÑà?ý¯3^Ò@ Ü2ÆQ¿ïÿÀà/€ ?î.-À,«Z?ìNÛ?JB¿Þ…pí¨åg¿çvFŸ¿à)¥÷ÞÉAGNbcuNVSS J120111-033219?ïé"Àšì?h‰ZÇck?fÝ?eá^?h‰ZÇck?ïì²µÈSX?)¸¡Ž¬?cMJ7¬§¯?)¸¡Ž®?ï…S•=ù?ˆW/؛?Ž«¸ðà?ˆW/؜?îVqÄë?™Vî¥û‹Ö?ª˜ïÓ±OÙ?™Vî¥û‹Ö4FGL J1201.7+1429?í°š¿ø6@R7UqKœ·À:'£.mѕÀ<'ÌK@!'Mš¾@oªÛ
}2?Ó?ÅíhN?םÊD\P?ýS'i#°@×Ç7a–¿Öùœ#6»Ô¿Üéwލ¿àѦPaAc¿êC¡É¿ïÿüÚ±'Þ?ïÿá∠ÎAGNbllOM 198?ïӒmaÔI?€­vY_ŠÀ?v6ÉOÛì?€­vY_Š¾?ï÷M øµd?h¸–2Ì:ø?Qd¾•:g?h¸–2Ì:ö?ìc½ p
™?¦6"±³i(?¼âü"<?¦6"±³i)?ïw¥Ú"	?'€ctEX?'KD­žá?'€ctEX4FGL J1202.4+4442¿ÔI"*mš5@Qw#x«‰À;7˜ólÀ<´"!Š"C@§§·§þ@xd"?Á]m
¦‡¿µsd%Ä`?ô
®ñð@/!Û¬º¿ÚícV˜¿ê"›Oe™¿ßŶƒ	_O¿çCO¢Ý¿ã¹Ë¾.ú>¿ïÿÿ)@k*AGNbllB3 1159+450?ï÷ȧo®?P¬tGüp?Pn± £Çî?P¬tGün?ïóÙñ5Ü?u'ÀoҌ?XMÂ"H€?u'Àoҏ?¯¥¦?‡gîØ?ŽÙT–V?‡gîØ
?ï¥fONà?w@ƒä¢?†¦l,zÈ1?w@ƒä¡4FGL J1202.5-0528?uÄ(:Ð@K©›ý÷èÀ:+L''ÙÀ<;µ%ç@[§c0ÑÚ@OãÖԎ?Á¸v¾ù$š?Áâôq¯›?öcLŠÅÁ@ztJ»?ïÿýaw¿çßlâj¿ê˜"t¼j¿êzª@/ðÞ¿ïÿv}_Ò#?ïücÈý4tAGNfsrqPKS 1200-051?ïþì¹ZÊ*?-Èá ©L?!4jS]J²?-Èá ©%?ïýGú ?M* Vi~?7ÇP/±?M* Vi€?å"‡?†	»iôQ)?‡Z†·^Z?†	»iôQ,?ïþ1Ý­ç?"#/#€ÃÀ?,â%&!Í?"#/#€Ã¦4FGL J1202.5+3852¿ê¢j÷°†U@Rœ;÷'jÀ:h/"BAÄÀ<'{ZqÍ@d[ô@ÈÒDŽ?µg×)È¿¬×ä>Œ
?õD5¹ö0@¡$29c#?ïÿíáoq'¿â£Éh">¿êsҕc©ô¿àyÈþáòÏ¿ã=š)âQ™¿Áù CVíAGNbll3FGL J1203.2+3847NVSS J120257+385147?ïöØÁƒ$—?TET¾ÏÍ?RN|ù¶Ò?TET¾ÏÓ?ï÷»at²?lêý	^Ëí?P‰=ӝM?lêý	^Ëï?ïÌ5QJ?wzËö‹)?yåWZöô—?wzËö‹)?ïžãŽÌ•¶?y† ˆôÉ ?ˆGLڒW?y† ˆôÉ 4FGL J1202.9+5141¿ÑvBw"²@Oå¡ÊÀƒÀ;CZPÀ<¢¬k-u"@O€íl@'¶'!%?Á"íå÷K¿´í¤ˆµñ"?õÕÛiGÂ@]Öÿž?ïܲø¿êbÑñÏ»•¿ç¿:¨rzq¿á×¼_AY¿æ¶ÇÝyÃ:¿±?štµßuAGNbcuTXS 1200+519?ïïâ|4Á?X!žÈMØì?`çƒË>Ð?X!žÈMØç?ïäÉ#Ýu?"¯Pz?k6ëÜ"‹5?"¯Pz?ﻡŸ§oa?{Y=9C3?˜$(	?{Y=9C)?S@¥Õ?€¨‡ø~Ð?Ûk/֊ý?€¨‡ø~Ð4FGL J1203.1+6031?µÈ¿~2@Kη#îÒÀ9zû¾QßÇÀ<o*þ±K@vò	óï@n—Oß;?¬èÿ¡?³`ËqØàV@^—eóS@	'R á·k?ï7Ÿçòm¿àBD]§ûÝ¿à'Y«m´¿á*i*f¿éV[¡'_¹¿Ð¥ÁۂOAGNbll3FGL J1203.1+6029SBS 1200+608?ïïÏ+¢Ï?X/P'''§?`b0Ô]0h?X/P'''§?ïÜ™37?ŒŒ¡f‰L?qÀ3yæe?ŒŒ¡f‰J?ï¡ßâ…ã?…Í5G•­?‡ˆ~ž‡G?…Í5G•±?î«]]÷ق?Ž.öKºÃ?¥J* 'gÓ?Ž.öKºÃ4FGL J1203.3+1119?Ú5å%'É5@Q¤_ !¸À:ç²7PþÀ<oIÊFá@7½%•ç@9'åøí½?͎8½`É?ÑޚTª|@iåvç¾@Ú¼ñ?ì[²BÝË"¿â¿ˆ¬Œ%¿çŽx¾­¥?¿×ž·æ‹º´¿ïÿù_|è3¿Áœª2AGNbcuTXS 1200+115?ïî7¯úÔ»?cÜI¬ÐG?aÈP+Eq?cÜI¬ÐI?ï÷}«uµ?a'{3}éØ?Q©ԖD?a'{3}éÝ?îÍáH‹cé?—
­5:ÏÃ?£!ëwIÁ~?—
­5:Ͼ?ïDµÞζ/?'Œ&RO6?—iD&):?'Œ&RO64FGL J1203.4-3925¿çÒv@6'‹â÷±}À:?Ï)è1À<INiŸ
@!*øé‹I?üב#'?·IӞ"?p?yùø²ŒbW?Åù çÁÆ@BÝJHy?éj‹#µî?䯂~õÔX¿ÞÀù"æ¯!¿á£œ*Øò¿ÒÜÍ Öy¿Ðå×?—ožAGNbll3FGL J1203.5-3925PMN J1203-3926?ïåó‹ctn?cú°Ö
J?jtœ‹Ù?cú°Ö
J?ïüÜø­}Ã?T_Ä6P?9:"ãþ?T_Ä6R?ïÓBhàq?yêi\@Ÿ?v^ˏÇtñ?yêi\@¦?ïµòì%[N?r—ßr??'ƒDö©,?r—ßr@4FGL J1204.0+1146?åUÔÖÈo@QÂûÒsÕ»À:w<
rIÉÀ<a
ž¿s@ ž^/‹2ù?üƒŠ´#ˆ›?ÄE´£ú?ÀRb"‰î?þy*X™J@
¢î$î¿ïÿýaw?ïÿþBe«+¿á1õ°ñ¤ó¿Ö¸_˜1¿Ù×i]ç'Ê¿ê0S'ˆAGNbll3FGL J1204.0+11441RXS J120413.0+114549?ïú^¿§"C?_yäÓmH0?F…aîîƒ?_yäÓmH&?ïôµ/•Ó§?qh6Â÷Ö?V• ÔX±)?qh6Â÷Õ?ïËZEp+?}]ý·ˆQ?zrRÝGêØ?}]ý·ˆJ?ï%€HH'?ˆû²Æ˜r?›OÿVöíæ?ˆû²Æ˜r4FGL J1204.2-0709?ïÝÌ1ímÆ@Jî`RP/À9nsbÎ+À;ÿ;"G@çß†Î?ü«åÌx7?µ#	ðCÊZ?µ—ÈAíá@.º'®›@—`,'?ïú·‹òçê¿äa©0'¿ßÝB»¼Y¿ÑÀ· jÄ¿âå4!Å¢Œ¿Þ•P^½$¹AGNbll3FGL J1204.3-07081RXS J120417.0-070959?ïÿqX‡à?0ÝÅç†?ÔïÄû?0ÝÅç‡×?ïùªMŽ¾k?[€,µ¸;#?IVÉÅT?[€,µ¸;?ïéðz…ðð?n­ìü¯5?f…zþ?n­ìü¯A?ᆱXæª?jGÎáÆ®?€yÕ)ÆU}?jGÎáƯ4FGL J1204.8+0407?Èú<Di@P7!Õ<ÞÀ;?ÐÐgŒÀ<~ÐV©Z@xB÷¡aº@ØÄ$"õ?Ðú? Ò2'?»æ;èך?èýpÇZ@	}=*WíR?惠žp˜ï¿êÉüÙ´¿â~wiÃèø¿ç5Š€Ìï¿ïöþdŠ¿ïÿñQçSaAGNfsrq3FGL J1205.4+0412MG1 J120448+0408?ïþó§¦^?' ëª,ãÎ? Ņš¨;?' ëª,ä?ïü2p«ÙÂ?Tõïd‡?>lz¡1ãK?Tõïd"?ïÀÈUþ(?I6С?›Õëþ)?I6С?ïç)¹
æi?UªWY?hÖFò•ú?UªWX4FGL J1205.7-2635?ÇmXÙ\@A"÷ µíÀ9mc¨FÇÀ<$
­,*@@SÃ÷f(@¥­Ûp?¯—d53¾?£9F? ô?ñ*MFðP@
cÒÃù"?ãR+Sk¿äå^ÿiؿ跍¹ç¿äNüm¾I¿èñžBuÆ¿â¸Æ báwAGNfsrq3FGL J1205.8-2636PKS 1203-26?ïïSN+?W«[v]®?`¬ç±ÔûN?W«[v]¥?ïûóhö'?Ræ֌ɩ?@2_ˆ%ø_?Ræ֌ɠ?ïÖ$Ï.2?ukg|…ܾ?tíû˜hç?ukg|…Ü´?ïìBĔÍL?R5È£±?c½;k2³/?R5È£±4FGL J1205.8+3321¿Õ¾7©¸@…@S—àÞ҉À:êj€§ZLÀ<'Æp'9S@réîñÐ@
þ`Ï6?Åhî
¿†ý±Wa¡í?À"‰õŒ´"@òý
':¿Ö® ¤»5Ì¿é9ˆ·Ê¿å½Ëb>Ž†¿ãe"bøô¿î	܍40‰¿ï½ A"ôAGNbcu3FGL J1205.9+3315SDSS J120542.82+332146.9?ïû@A(?AI#L™?C²ÿâû`(?AI#L™?ïüñ&ûÙà?T­7ç?8vÈ!0ûÏ?T­7ï?ïêϘä'?h·‡<²?e0gá}¢?h·‡<°?ïñ†—ðÑ*?MÁ'¼Ei˜?\òÐ]©à?MÁ'¼EiŠ4FGL J1207.2-0524?í¨sÃ/ëN@Kàw¯dÀ;ÜÂä¿À<œ¤ÁëÈ;@ ™o¬5R?ù-Æèk?֒ÐÝR«ô?Ý
³ö«˜@x÷…@±ü/æÍ¿ìNá¿Î¼?ï{ìàh‹¿Ñöã•Ò¿Ó>úç'Jñ¿ß='üft¿ðAGNbcu1RXS J120722.5-052442?ïû)¿È7?Eœj,Ÿ¹?CY݋$ò?Eœj,Ÿ¯?ïôY R?1?kËÍ°˜ÉV?WL¿[é?kËÍ°˜ÉV?ï]"ê?ŠdUû?ýtObÌ?ŠdUû?î÷
mUì?‹æ݂°ÙH? )*¡?'?‹æ݂°ÙH4FGL J1207.7-0106¿ÚÐnˆ®Ø@Mï÷øʂÀ:"ºˆýj$À<e*F$§@Î]Àz"@ÇúBPÝh?Àø==ù
?ÆÚ9ÝFl¡@ŒXž&Ç@éÉl|«?ïïZ@hOö¿ÑiدY¿ç&Zݜ'é¿á"?B
;˜¿é>ê¡tˆ¿ðAGNfsrqAT20G J120741-010630?ï䗒òa‡?l»ãJ"¢É?khm
žx?l»ãJ"¢Ë?ïûÏLÕ~1?R›"ö%I??@Â̪7Ó?R›"ö%IB?îKŽLàÉ{?›Áã]v›w?«G1óhR?›Áã]v›x?ïü({Fï?-© ÔYj$?>¼'uȀ°?-© ÔYj%4FGL J1207.7-2229?åH&'ƒÚ@C£vfœíÀ:[§ºÄŒŒÀ<e¬9¯@DÛ½€?ÿ¾›ÌyÀ¶?Á7°év?±ô¬¶¬Ð?ñãUŠv(@Š`Á‹Ñ?ïÇ~¿M³<¿âg1g™¿ãåóö¿Ûp°½"Û¿ÞÆwž5@¿æèþ[»AGNbll3FGL J1207.6-2232NVSS J120736-223036?ïþ-Oã?$Ã龜Œ¥?-/ÁÐ?$Ã龜ŒÕ?ïýö\>?Påÿrbž±?7hOå	?Påÿrbž´?ïû®~*Œç?S¢î¸Œº?AFUÌd$?S¢î¸Œº¸?ï誗ùÚP?Pj{LŶR?gUh%±?Pj{LŶF4FGL J1208.1+3017¿î9áÆg @Sÿf¥P‡À;x+¾Ê«ŠÀ<Пe‹u@!KQŽ½ók?øœ bv?Ô\™`?ПäâBTä?ùÕ¢y<,@\<ŽÑ"ˆ¿ëÀnºÈ¾J¿ïûmÊö?ÒÊM8ßð¿Òk.óŠ§¿áì^Á¿Ô1»¬éØAGNbllGB6 J1208+3015?ïúñ5É	?H€¹Ÿ¤G?D;Ó(Û×å?H€¹Ÿ¤[?ïü¦0ŒÙë?QÖâ'ñ<¾?:Î{™0§?QÖâ'ñ<º?ïÝïþo	Œ?qĵ!?&?qÈ{9Ë?qĵ!?&?ïÞî9÷=n?_ÿÂnû?pˆãaI4?_ÿÂn4FGL J1208.2-7810?âÃ8DéɍÀ/d"À:¬#Ï!kÀ<hýwƒ–@ =÷¼d ?ÿjj6Õ#?ʳiäËG?³Ÿ€ŽZÌ)?éõv¤¢X?óŠy?­¿å2 -"¿çâ/jPÖ²¿Û¯~ˆF5¿Ûo/BÄ#¿á@¤Ö
¾/¿å!	ۂrAGNbcu3FGL J1208.2-7810cPKS 1205-778?ïüü*M´?5ôFÚ+÷?8–­'c:?5ôFÚ+ÿ?ï£ôhe;Ž?˜¦îÇ&R[?‡å汘?˜¦îÇ&RY?ïçÓl²,?q€a@}j?hb,"MÒª?q€a@}m?î%á=Ú$?\‡úgd?¦ý¡ì"]´?\‡úgd4FGL J1208.4+6121?ï÷w)ëÂ@K'BZîc À;Gy;UAÀ<ãÚ\ØH@þèL/-•@ü÷¢cl·?Á±Ýˆ0æ}¿£ýÛb'Ő?á¨áJÞ @	·ïEÀ¿íÜ3rSοÚ\uâ/_"¿æoÚ•[œ¿â,ûv-ƒÇ¿¨`Ž­K ¿ë

"ZAGNbllRGB J1208+613?ïÿž³<?";žrmö?,)˜ß©?";žrnB?ïýg™ØL?NSDÞàZ+?4Ã1=›{?NSDÞàZ%?ïîŽÐ™?q)ÊfXÿ?aq/fpã¾?q)ÊfXñ?ïþ@y<g?!6þÙlĎ?+øn\9÷?!6þÙlċ4FGL J1208.8-1751?ïNŠvÁJ@EêÖ¡aä÷À:ë‡ß\òIÀ<~ϙ/çN@x¤ÉM'X?úøihyf?ئးø?ߚOa'C@I	¼AdN@JdJ,sü?ëÈì}—/‡¿ìWàðñ¿ÑƒÞÐZv¿ÜgŸKŠB¿î]UE¬²¿ïÿ韖]ÐAGNbcuNVSS J120856-175647?ï­)ó4{?xZ‹Ö·?"µƒ2ýá|?xZ‹Ö¹?ï­Z!l?²G˜ExÓ¡?ŠT¾;Ҁ?²G˜ExÓ¡?í¨J'V?¤~Y']‹?·ÿj½«mE?¤~Y']‹?êϤ|ƒB?¬+<`¦:Õ?ÄÁnéòù?¬+<`¦:Õ4FGL J1208.8-2754¿êšÿo~µ@AԀuÀ:œ(MüãÀ<añvÐ@ö@ˆÂ‡y†?ü~†ƒ<`?ÔS—VÉ:q?Ó#ç{NÕÑ@Ù櫛#Ý@é?'³"W¿ïÿŸ½ 	?ïî'ð2,£¿ã°E!óé¿Â½§€b¿èÎÁŒ&ê¿ïÿüoQÇsAGNbcuNVSS J120900-275350?ïØDõi&?xT]²"J?s݅|KlÝ?xT]²"J	?ïð&9^?}®KhLpD?_߳׍D=?}®KhLpA?íÞ[ïO	
?¡bjc6†?±
 …‡·˜?¡bjc6‡?îÁ9ˆÊ¿-?'p3Wç­Ú?£ìgsT
;?'p3Wç­Û4FGL J1208.9+5441¿è'€4³á¶@N­gý?[`À8¼iuå_kÀ<Bá³
Þæ@Œì‡¨*@é»ðÜw?¡$åhd1?²·z«ð@`"~@'¤¦½ïd¿Õï5­`÷¿äþ'"o¿çñ¢4rοæñùý‡¼¿î™pI>7s¿ïń~ªTþAGNfsrq3FGL J1208.7+5442TXS 1206+549?ïüy{4*k?4N¶j]I?<4&^¬¬Ì?4N¶j]5?ï÷UûÖ]|?ibï'§VÅ?QTSE_?ibï'§VÉ?ï—4k‡;H?ˆO8µ²5÷?Š2å1-þ?ˆO8µ²5ô?ïüjÛ'ԑ?1ò¹èñâU?<©&Á[vd?1ò¹èñâG4FGL J1209.0-4630?ïìS@¸–D@/~ÀÖõD»À;"G¡A)À<`émƒÐ@0\"*š@mgâghÅ?ÍçΰқC?£ÝT Á?ٟ"ÛCÝû?þ›©¡¤ý?è,ck	cV?ÍYþí[c¿ë7»ûS¿Ðzý©8ž¿â£Ÿ¬Ù¿ïá½?6.AGNbcuSUMSS J120905-462944?ïÎÝ»Ò?îA5~r¾?x'"xð–¨?îA5~r½?ïq=û=t?¬Gû±\âj?'Ø@˜Qp?¬Gû±\âj?ï^Û¬ó?•´ÄÚ;?"$œÊáŒ?•´ÄÚ8?ï–]l8±¼?v…b™?Šh¤ñӑ?v…bš4FGL J1209.4+4118?ç'Æ_@RY•ÔèûÀ9¯¡BÛGÀ<N|c'í…@^owG?ý¥óå?ŠZ?´åp‡§~µ?«Û^¸r?öÖ»cý@]–ý]
¿àˆÊ>}¿ãš:Þù;¿à›T\ÈX¿ÐÜÍ`pƒ ¿áf¬ƒ§À¿ê†#À¤ukAGNbll3FGL J1209.4+4119B3 1206+416?ïü¤ì?9™˜ÛÝ35??â؟ÈÔ?9™˜ÛÝ3#?ïú
®ßV?d«G°¨Z¡?GËÅD'¢ë?d«G°¨Z¨?ïì:.ß~?rÉÓvÕV?cúÅÑ '¥?rÉÓvÕW?ï½Ã#4Óý?lYn{5¦?€72Ë?lYn{5¢4FGL J1209.4+7608?êð¿P¶üq@D\Fà!qÀ:¼¼Š_ióÀ<Ön%wˆÎ@ÿ˜Î˜~ç?üñÊ,ß\?ʃ2yúÂÔ?Ói¢À^Õ@YíÚcŽE@	PålU闿ìëF…¿ºõ¡Aٔ0¿Û·yT¼¿Ü_G£­™¬¿êñ0š¿ïÿJ-J»æAGNbcu3FGL J1209.9+76072MASS J12093020+7609120?ïñ¿›µ¹?]ؾ\Ú}?\€È•þŒ¼?]ؾ\Úˆ?ïû]ÆOñB?X	â-í?BˆæÀ:û?X	â-ä?í!wa½?¤=°'™Wò?·nôDòV?¤=°'™Wô?ï¬^Bæ×k?qŒ.=›ì?"èoFJ%n?qŒ.=›í4FGL J1209.7+2548?Õ½¯"ã¡@T%sBí»ZÀ;|iÃ8èÀ<Õªøg…@1<¼ô½'@9±Y©¿'?ÑŽŸÀz.?»G‹.ò±¹?çÀÞöÅð@Ͼj´SÚ¿ïé‡þ'•ê?ïÏ[½•ø$¿Ç÷D…(0¿Ù·ª%ØØ¿ä?"=ßßy¿ïñ/DÀ#AGNfsrqB2 1207+26?ïû¶áùrj?<ž¶=?A$x6X°?<ž¶=?ïø¸"¦?oi쮟?Mu½g¬½?oi쮞?ïÔ²à%†?yŽ¬tÈ«?u¦øí<«?yŽ¬tȯ?3—ò?y–VH›yÞ?‹ßà3m?y–VH›yÜ4FGL J1209.8+1810¿é¿T¾½`Ý@S9,{‰
ZÀ9•8¬øÀ<IwëÉè@&ãÏGÑP@'ìB³Ù·?°–1Só?™6&`D–æ?å—4àh@i$ ô+á¿Í{.I"s•¿æD}ˆkõ¿å¹î£·*¿æe̽ÞGt¿èvuþ	ῼß0Q¬pAGNfsrq3FGL J1209.8+1810MG1 J120953+1809?ïü¬0'4Ð?0䦊Ÿ@?:ž{vY©?0䦊Ÿ?æ?ïý;MÄ?P'lõ"?7ó~%'âl?P'lõ.?ïæ"Œ<‹?h•¯Úª?iÝsÃtìë?h•¯Ú²?ïÿfû~ó?	ìW¾êº5? =AŸ¯?	ìW¾ê¹Û4FGL J1211.0-3800?ÝÔ·ÝÒ)¨@8,aՈÀ:`~XËs0À<b$Óš@ð[Œm·@¶ûú·Á£?Â1²)³W±?Á2Ã6K¨?ÿ"Sd+"Ã@ð™§0†?ä±+¡nz1¿Ò·6B\Eü¿å;ÔÂd"¿ÞC5ߵݝ¿êðj`Æê5¿ïó‡K¹;öAGNbcuPMN J1211-3754?ï¾Å´J_3?€'XՔ­R?€N'íh35?€'XՔ­P?ïùjÜS™Ñ?`j+ƒóP?JTŽ±˜¼/?`j+ƒóP?ï…
Šƒ?ŒbQÔ/#Ñ?Ž¼_9F?ŒbQÔ/#Ò?ï{w©OÕ?rYÈé9~?Œ¡"¬
õ?rYÈé9y4FGL J1211.6-2735¿ïõ%W-Õ @A: _ñØÀ:?d?D¹mÀ<‹h~n›@@ï3@WM>w4?Áï$»v8A?²j(gÓ"ý?ïˆØ¡lKÙ@
©;×òp?¬˜¾A2"¿éµ\8;¿æçKžd¶¿æ—4d‹šÓ¿êoÔ;V¿ïþ§¥Ë×AGNbcuNVSS J121135-273615?ïù«˜Ùw?F
Üièz?IQœš#ø•?F
Üièf?ïý3Ât‰ç?KçÓb;b?6aì[°Æ‰?KçÓb;'?ïו$sÀ?tύ‡cD~?t5mÆûˆ?tύ‡cDx?ïéGÈQªw?TZ¾b
?f¸7®U‰¨?TZ¾b4FGL J1211.6+3901¿Äù,A+»Ú@Rß`þG™À;Yá'nÀ<ÞÖÜGª@î',èÁJ@ƒœØ{?ŔS»d¿ª?ڜªVf?ä UàÝ%
@-=ÐÆ?ïÎá£0ò¿ëbS².»Õ¿ä+z!"4-¿Ùô¼ .ß¿Õ'äKn"\¿Ýõ3ô#RëAGNbllFIRST J121134.2+390053?ïý«/3NK?+6A²'G?2¦†e¦2?+6A²'?ïüöwZÔ?R
™¶òý?8LE)_U?R
™¶òñ?ïûÁJQÉ?A–Þ¢Ó?CðúÖ¸åí?A–Þ¢Ê?ïõZÀÑý«?DÀgçõ<?UJ~\§Ù?DÀgçõ<4FGL J1212.0-2326¿åÔ}ø©¿@CDQ£"îÀ:_bnŠ!WÀ<N>Ȓ«i@ ²WlÎ_t?ü‰ý_;Ϻ?Ĉ°'Ð~ˆ?»ã8)‹À?ùÎފdrp@	³l`%…?â}E`1n¿Ýy]¹ïz¿âLuĨ;¿ÐàØóK½¿áƒè¢–Bw¿ÛX£Ó¯AGNbcuPMN J1212-2327?ïþ½™–˜?äªkŽ=?$.æf–~Ú?äªkŽQ?ïýÀY–Z?L‹R6£&h?7ùý3M4Ñ?L‹R6£&g?ïìČ)sF?s}ã9î?c;s֌»2?s}ã9ô?ïë v'j³?OF%ëó¯?d߉n•M³?OF%ëóÍ4FGL J1212.0+2242¿°Þ©–U]1@T½D¦"À;1	G|À<Ã"̳¢@‹F©\°/?ÿw_²íþ?ÆòT†?Ï?³ˆÝðǺ?ëöŸ™Û@ÓêÎ?"¿ïÿE€Þ$?ïö?ŒÝÉt¿ãI=Š¥
¿ËÉKãÙ-ٿꇥïaL¿×+¢zé«*AGNbllRX J1211.9+2242?ïõÌ
Q/Ê?P²2"NA?Tgå] i?P²2"N??ïöX"Qù?lƒûÏû?SÓN×\s?lƒûÏû?ïƒFÅbÍ?ŠÙ
Xt{…?>îN§LÌ?ŠÙ
Xt{ˆ?ï0³VÝ8ô?Š•™ð¬G!?™é•$Xáx?Š•™ð¬G"4FGL J1212.2+2442?ï¸ØCµ,@T6éNã'âÀ:ç{³Õ…À<¶tðlå@?EbŠ¹­?þñ
‰U~¸?ÉL'jPUÙ?ËÙ@x–Ó@'åøí½?þkÌ´Îÿ,?ïŽBî's¿é='þ¡±¿ØëxßdÔì¿ì{Ô!Tä^?ÐZ"ŸY¢¿ïþ"ØrAGNbcuNVSS J121219+244130?ïï&Jô|??cê¯Y—"?`ÙµƒÀí?cê¯Y—•?ïèÿç¸?¸åBðžw?gèçH²?¸åBðžx?î>aT?ŸÉçDý?¬)ê¶/º?ŸÉçDý?ï(	ig'?–çâ'ØZb?ŸÚþÒÓÎ?–çâ'ØZd4FGL J1212.7-1402?ï»|8šh¨@Gã1üÒNÀ;lk§îÆóÀ<¦®òÇ2Y@ ߪG;Ô?ÿø¶zzða?Í&"©x3î?^ô¼kZàÚ?ý©t"$à_?ïŽ:ºæñ¿Ö¾"š´¡³¿ïÐéÅ?áý'aĖ¿ãˆŸvRl´¿ÞØ⚔kAGNbcu1RXS J121240.3-140141?ïýª¨Ïæå?6šy³øá2?2ª¹€ÈÙ*?6šy³øá=?ïö'Þˆ{ö?jì_ú…Ùî?RúBïõ?jì_ú…Ùí?ïà·°õh…?r¿¥Há¸?oHO
—{J?r¿¥Há³?ïÞòyѪ?eËL'K^?pýÃ*Ä?eËL'K[4FGL J1213.0+5129?цˆÈó3@P%˜Çâ'AÀ:jQ•ôÉkÀ<°!èˆ6@aþ÷KÑ@pÛ4n?·<? |LW¿–¢÷Äг?Ú¤ÐÚN@ýŽøUç"?ïDž/IŒ¿æq*_Oð¿äÊìB3]¿ÙûÏdÛr¿ã@TN5íù¿Ù"-Qqâ›AGNbll3FGL J1212.6+51351RXS J121301.8+512942?ïîÂÝJ?V3¸ È´?a€="¶2?V3¸ È¹?ïý#$.Ë?K1‰wŒò?6æß։›Å?K1‰wŒú?ïê1mš?sz?œÁ]f?eíÎâ'f?sz?œÁ]_?モnd¥a?h­Æ³êD$?€[$fÖ§°?h­Æ³êD*4FGL J1213.3-2618¿ï&‡]Vÿ6@Aãƒ'gMÀ:gn³<À<U£Ô…þ²@!(GœÌª?ùmóXQЭ?È÷V¹Eë?ÌÁïy%µ@@~$É
%@ÿ¤åÄ¿ïÿî' Ç?ïÿÑa\w¿ÝÇyB=?)*sqäT¿á…¤O\_¿Ù+¡ƒóÀAGNbll3FGL J1213.1-2619RBS 1080?ïò©V‡št?Ww}ô_2­?Z­RðË@?Ww}ô_2Ÿ?ïùËâ6?]q&e˖?HÐw'¯–7?]q&e˦?ï@6ôU1?'«2ªH?—ïÙ!uYã?'«2ªH?ïxAÀ*']?AµˆÛ©<?÷Çú¯´w?AµˆÛ©C4FGL J1213.6+1306?ËïØòšÅI@R[Ÿ@¢‡À9·ð†nDÀ<.z>å@mï@Ec#»Æë?¶oè›4y?Èì$+@Ž;—…Ã?û,;rFïS¿º)ß!Ž5¿à_¾ÿ"°¿ãΈŽ¯Z̿ꮊ!V'Ý¿ç"ñÿ·/Ø¿ïþàEO•jAGNfsrq3FGL J1213.7+13064C +13.46?â=Ç"ÑÃ?ʞ+Ê1?ۄqºà\x?ʞ+Ê1?Г%žú8?Ó¼—'Ö?ç¶m0ðä?Ó¼—'Ö?ãֈ—BÁ?¶µúmùñ@?ØRîÑz}û?¶µúmùñ@?Ð
an;?¶²''|­Ý?çùO7Èøâ?¶²''|­Ý4FGL J1213.7+6423¿ç*PÕ`ˆ@J9C¬ÅÀ:¿ØCùTÀ<ȍÿ1£ç@3ʗé@K@Y|´†…?¹:üUP"m¿±™Ö?è"i?ö'ÄãÊ?T@
«‡WÎ?áM̧
£¿êŠ~¬-p¿áÌs`ŸÒï¿äÏ:eV›î¿íOÐÂû'³?à$"3ÿAGNbllNVSS J121348+642524?ïö#­'?P‡p*Þ?SË͸¤ýŒ?P‡p*Þ?ïüP¢+Þ¯?T¹Z¶?=zî¡
€¨?T¹Z¶?%~Ù¤?ˆ'°üĸ'?ˆX6 I—L?ˆ'°üĸ'?ïïp"º'¼?Q©JUçbò?`ÝEØD"?Q©JUçbî4FGL J1213.8-4345?ìlLðí@2—àXšËÉÀ:Jr}ËÞÀ<%)Wèb@ÚøžaÕ]@¹cc}?Ä[ãÁn?±Ó)]F'?î0kؖ/?ú¶[
í©f?ïðØïÿ¿éÄÌîZ¼¿á6sŸ_l¿ä‹«šM¿àb‹"¿ïÿýawAGNbllPMN J1213-4343?ïîÿoHk?a±ƒÁÑ*	?a·"áô?a±ƒÁÑ*?î¡I"@?ºÿQ˸©¡?¥ëfËþ?$?ºÿQ˸©¡?"¤u´?‡Ÿ,'‡ÿ?Œ^Öâ'û?‡Ÿ,'‡þü?í%›ºO:4?ø"k?¶Ó"-†.a?ø"k4FGL J1214.6-1926¿àIÆÖJx+@EJ8Ÿƒ¾fÀ;;÷'À=¢ÌHB@ài4!Ö@€\FQóé?ؼ‰ˆª^
?ïÿõ^'@ÌiegÊ?ù…hŒ,¿ïšÇ‰W'?ã¨	3…hŠ¿Ö‹¥»ç¿îD´š¦ßÓ¿èB½—¥¤¿ïÃㄟ6'AGNbcu3FGL J1215.9-1926PKS B1211-190?âͬ½‹û?Ñ#]@?Úd§ö"è?Ñ#]@?ÔFc/ò?Õ.{¹æõß?åöÜÎh÷?Õ.{¹æõß?á0±»Ãç?¶æ@v[Ú¤?ݞœ‰âx1?¶æ@v[Ú¥?¨9®eÇxÎ?"^žå[ë?î|e£ˆt?"^žå[ë4FGL J1215.0+1656¿æM˜Åƒòj@S2œ#·•-À9x™sÙìpÀ<C?»òn@ÿ¿¼îÞE@!	!ç±U?®ôA¡?Ÿ|æ
C?êêú~Ù@'³{"†¿Ð/Ú¹š¿ã ^l¢¿å-¿öût€¿æ,£ÌùBw¿é•}
Ú7¿Ôe™¢Rû¥AGNfsrq3FGL J1215.1+1658TXS 1212+171?ïü'ý)·?0em³@©?;pö²=]?0em³@ª?ïüÕ¸ôçÈ?RCWÏ-Ÿä?9R8XÁ¾œ?RCWÏ-Ÿñ?ïàŠ¤c}?q$Ø?÷©?ou[œé'Á?q$Ø?÷«?ïÿ¹Ã
!>ø}ÉiÒ?<·½Xë>ø}ÉiÌ4FGL J1215.1+5002?åLéâD°@PƒcÜHjÓÀ:†…ÀŸÀ<sŠƒ| ã@ !¬zúÝ?ütA…ÜMs?¹ß>>?³kAþŽL?úâ$íö@@	f†ã¿ë…e?IìÞ¿×f'|E˼¿à.jáö)½¿Ù~˜¡ÌîׅܿÜz>à¿è~ú1‰æAGNbll3FGL J1215.0+5002IVS B1212+503?ïóñÓõî?SaÏáݎÇ?XxœX!Í?SaÏáݎÓ?ïòݟ`À<?p÷¥¤XÈ¡?ZDÁ>‡?p÷¥¤XÈ£?ïÎÍhúm?y,šÔ¬‰?xÿK'ÉW?y,šÔ¬‰?ïBn•'5¶?ƒ"¾5Œ4?—²-O¹I8?ƒ"¾5Œ44FGL J1215.1+0731?Û±·Uˆ©¨@Q%¼¾aÏÿÀ:œ¥ÛÇ;"À<k
€òç@!OŽ%óÃ?û/ã7r]?¾9 PB
?˜0':±š?Ý-o|@5ÜiM¿ï¥˜Æï¾?ïã€}"Ô‰¿ÝXcg™¿Æð»ix¸¿äw,ò§Q鿾yĒÁ³AGNbll1ES 1212+078?ïüË°w8?7½v´IÊ?9¢|F?d'?7½v´I¦?ïúcpMY"?\ÈÙBôJÝ?Fr>ʙ²Ö?\ÈÙBôJä?ï鷺;gí?dŸi…ȵI?`[EĘy?dŸi…ȵ>?ïË]š‹?l¶?¼È³ô?zQqö²»R?l¶?¼È³ø4FGL J1215.1+3513?ވCœ+ë-@S³Q¬šþÀ:׶6ˆRIÀ<–µI"ˆÁ@Îbÿÿ'@<ewS?Æ¢
S?ºÝzÐj?ð#	"ãÿï@lÿGµ¡?ïýl!'J@¿äž‹`Æ¿B¿èúàŽµ:¿ä îzÔ]¿ïø½KO‰«?éÓÈ3àØAGNbll7C 1212+3524?ïãyë7ox?ró'ùƒFx?l†Ȑˆ'?ró'ùƒFx?ﳄ;$E¹?ŸW÷kšFT?ƒñ6î'ï?ŸW÷kšFS?Y;ÒX?ƒ÷æéý‡?‹)±j?ƒ÷æéý‡?ïǔN5†?ñ=Jû?ŸG
v9OR?ñ=Jû4FGL J1215.8-3732?ïµD:6@8ˎ\NµpÀ:ØxFÜÀ<h)à¤&@o›Cgß@Ö¢óµo?ȕè41_ô?²
M`Ûâê?ë%ˆ M?þùr奶³?ïÝÐË_ƒ¿åä¶Î]Ç¿é®`Ðû0¿Ýgzbœ­J¿ÓK' Q¿ïþÜIA'rAGNbcuPMN J1216-3734?ïùf¬Ö]½?KÂ@ÃÀv?JeL¦‰?KÂ@ÃÀˆ?ïò‰ô'?s±3™H·?ZàíÞÛë?s±3™H·?ïá˶Lf¼?m$ÒXþ¸ì?n4I³™D~?m$ÒXþ¸î?#~È?u¢8Ï-Ž÷?‰—7 ~N`?u¢8Ï-Ž÷4FGL J1215.8-1733¿ÚKDcŒo8@F=Â;yRÒÀ:F¼—Ëc@À<H…7È@N´©‹Ó@ú0bžZÉ?ÂÛy¸Ó›ž?³Ffdÿ´?uøª¡@—EôÖ×?ïiæþÒ-Š¿ãã
ìQÍR¿æDڐå×ê7@Þí¿ïÿèþ†®/¿íÈÔàl'ÏAGNbcuPKS 1213-17?ïÏéh`ùû?yíã!w U?xKσÐ?yíã!w T?ïÔ®#=×?‹cEýd[4?u¨î8aÿ?‹cEýd[2?ï|ãž4''?ŠíڑW?cŒ9m»?ŠíڑR?î‹׀€?'D…-Ĕ¦?§N2‡÷î?'D…-Ĕ¥4FGL J1216.1-0242¿îõÚx07@M{›€#¦ÎÀ; ÆÞvB|À<›'–FþÂ@ Ëÿ)@k*?þobð ?É'dÈ×tÆ?´¾¾l6à?îcâÞ1#9@Y‡¼ÍPU¿ïÿZ=¹?ïêâ—9m	¿¦IøŸ¿ä|â((¾¿ÄŒùM3e¿â=)¡dPAGNbll1RXS J121603.6-024302?ïýž@Eñ7?3]zĄ ,?3
ýÐvI§?3]zĄ :?ïüÁ Ç?PÌq²[ò?9÷
ÿQÏ&?PÌq²[ó?ï×"¼é=?y¨ê‹Â?tn¡ù‹`å?y¨ê‹Å?ïي=5¨?hOUíœI?s:áe+·ã?hOUíœI4FGL J1216.1+0930?ìh-èߞR@Q Õ{Ç÷{À:bSåZbÀ<|ërl.@ndD"D@#~Ýx?¼aU"9]?ªþ8C'$¢?ð×*à¼?ÿ†k5X'¿ïð'Úb·…?ïS(Ü¿Þ¨»àì>'¿ã™Á§Õœ¿äƒ×ûÔø¿¾éÀÎfÕÍAGNbllTXS 1213+097?ï$?^HŒèWj(?aã`_Ûÿ|?^HŒèWj.?ïìY	ß?u[Ë]~Ô*?cpå¦ö!?u[Ë]~Ô'?ï®ö"Êñ?''Ž
AÛü?"B\·MCÜ?''Ž
AÛý?î''j€¥?•´W½ò?¦Ý‰Wõ¯i?•´W½ò4FGL J1216.2-6121¿îÖèæŽÚ–?ó˜2ü¬ŽiÀ9Ü»‰®jÀ;(};•"@•þYŒ¹@͒Z
7'?Ðùn
Áà?Û¯žS<½ö@	¿v¢ôŒ.@ ÂèóI?åmíät‰?¿á}S³{j¿áÓçþ×`ú¿îO
`;¿âzm"gÙ-¿ïà‰B37AGNbcuPMN J1217-6113	?ã 7yë¡»?ÌÅÔhN9~?Ø¿'(¼Š?ÌÅÔhN9~?ØcºR!Úc?Õ°)AÝE+?ãÎ"ÖïÏ?Õ°)AÝE+?ÚpƑ'í~?Àfà.õõî?âǜ·>‰@?Àfà.õõî?Þ`c¼ý›ˆ?¾+ЅHúº?àÏÎ!2;?¾+ЅHúº4FGL J1217.9+3007?îǎê@Tƒ×Ûô‡ýÀ7ÔÄèÒ½À:ÝgD²·x@ýpÌÚ?ýªˆ>•g?'H]+?§¡—s¡k@6ï^Èt@Δ$9Æ?îg¬sßÌ¿Ùù{Óë¿Ýç‹z‰‰¿Þs¨£ø˜-¿áJ'Á¿Þç=[«!AGNBLL3FGL J1217.8+3007B2 1215+30?ïý³dƒK?+Œa²í²"?2dÛ㕱?+Œa²í²&?ïïÊÜ£;T?tò´4«?`5#\ĪK?tò´4«?ï´0x‹z¢?†=¡xðD?'óáÝ!W ?†=¡xðC?ïøâlß?> Å%
œà?LvLñƒ à?> Å%
œñ4FGL J1218.0-0028¿ëß4iŠ/@NŸa»úìÀ9ûKиê˜À<0=áÄ@b÷Æöt@26 M}a?»®ÌÒ|å?¸`ýµ'?ùhöHÇ/@	i
؅½š¿éã_•'Í?ÁríÒ¹K¿å^ïäÿÉy¿çՍ@öv¿Ú">þî]¿é¹¡KêAGNbll3FGL J1218.0-0029PKS 1215-002?ïíäm]þ%?fv™Ã#­?b'¢Ü
?fv™Ã#­?ïûX&Z÷ü?UöÚ˜?BŸf" 
á?UöÚš?ï'|›ê§î?FÎ>(µ?`ÙVO?FÎ>(§?ïÌTEÑ0»?jêr±Óçq?yÕÝg¢0?jêr±Óçx4FGL J1218.5-0119¿ïkšÍeÉ@N;gäçïÀ8ÞÚVùÀ;©É™;¥È@p¿#¤@-;¢m}²?¨n'>´Ï?¹3©û'†P@À2˜À¥@ÌÒÖüü?ìïÀÛå¿ÜÈ¥ߙX¿áéÄ[å¿áb©B"	¿äës`¿çôþÅwAGNbll3FGL J1218.4-0121PKS 1216-010?ïý@ûÃó?/gݪ#7?5ø'‰àl›?/gݪ#S?ïöãNTI?ev—Jæ¦?R9ÇcWkø?ev—Jæ¦?ï¼×xöº?"HX=5"<?€Ê!ÂQz±?"HX=5"<?ïæÚ«dfr?Ue`ö4Ðå?i%T›™Æ?Ue`ö4Ðî4FGL J1219.0+4827?á	¥«Õ@Pñ<64À;d‰èK®TÀ<¾©Ü¡V@àÕ:Y˜"@](¯Fª?ȤvçvF¿Š­ükå›?‰ö­›Ú@išÎM?ï`¤&ó¿æBnd!¿ê¯s?è£B¿Å
GÅwÄ¿ãît½A>¿ïÿf¢¡U%AGNfsrqON 428?ïøÇê¨<?[™±¶·?O˜àU_?[™±¶´?ïý³ÛH?MG
?3òa'Â™?MG
?ïÍK ?yÂz.Ï÷¥?yxñôÚ0™?yÂz.Ï÷¡?ïðiõk"m?OaÒtn©?_,)»("?OaÒtn'4FGL J1219.0+3653?Ûò‹÷¨åª@S…/D')‰À;oP–À<Îâ*,#t@nx‹¬ñæ@©A­Iz?ÓÀQ>a¹?ÖÇö8Öá#@÷P™u‡l@B8!°º¿çt]î$?îo^‡ŸÇ¿Ù£½l²†¿ã2HQ¨i@¿ïûñH¿ïë6ÊñUAGNbcuNVSS J121915+365718?ﬥt?šïœIÆqg?*k\Ñ|?šïœIÆqg?íÁvˆ‡"?Áº«Ñü¨?±ôK¿[Ãk?Áº«Ñü¨?ëÍēĚw?§
œ³Èî^?ÀÈí°í–!?§
œ³Èî]?åG&¥À?¹Õ"ø?ÕÑéq²´'?¹Õ"ø4FGL J1219.0-4827¿àBÁ¡D~@,#ÿï9_À:+3ªQwÂÀ<>J—ÓƼ@bxqÏ{@¹m	Ö¶?¼jgÒÍõ?ÊULù	ð@âÑ¡GãÄ@ï¾'˜uW¿ì	ì³!Ÿ?Èx¤&æI¿áå¢áìď¿àÆY`nº¿êÁ¿åԐ{æ˜AGNbll3FGL J1218.8-4827PMN J1219-4826?Øv]ÌÁ^,?ÌZP#"åÁ?ãÄÑŸPê?ÌZP#"åÁ?í-ïß©áî?ؖÈóçž?¶°ð"?ؖÈóçž?á»MYçæ4?À¦ñô°l]?܉eL03—?À¦ñô°l\?ë…nK40?£.QZnZ¹?ÁêFÓç/C?£.QZnZ¹4FGL J1219.6+0550?æcÓK¤˜@PÙ¼¾aÏÿÀ:êÒëʾÖÀ<–"
>@XÜüŸÜ?ÿ'ø½ì_9?˼#.XX?•_¼~?óF«ë«µ%@E9ÜœH?ïÁCâWùf¿ä.y$¯ò¿ßõ]¨)¿à{Áâÿ2¿äL-4ìp׿áÿÅGAGNrdgNGC 4261?ïý3Ç¿;e?4ûÙìe?6aÂ$Õ¯?4ûÙì?ïût̲Þ?Z·6{øî?B.Í4…õ?Z·6{øî?ïòĝ}t—?eal"nß?ZvÅÐM?eal"nÈ?ï·%'"íÏ?j0ÃY›à?'6›ZČD?j0ÃY›Þ4FGL J1219.7-0313?»«Ó]¬Té@MYµÜyÀ9õÍXãÆäÀ<7"U²¹ü@ Æ2ÿ±§?þL(²¦°Ù?¸DÛ&VÖÑ?§(ÍÂ?ñ
ÿˆ
ûÝ@+«	X™I¿¾¶x¢~¶¿ç
>¢¨!¿Ü'|ÉV¿Ü^-ØÖ¿á(aNcæ¿×	ýDcÝAGNbll3FGL J1219.7-03141RXS J121946.0-031419?ïý«Ïw"ä?(涽/T?2¡"FèçÇ?(涽.ú?ïû¿ßþü×?WËåŽê¨ð?A€¤¡?WËåŽê¨ý?ïúS˜ë¨?Jáu¹½ç_?F±œQ]ÅR?Jáu¹½çJ?ï㚦Âî?Tà› Íû?lüeY=_?Tà› Î4FGL J1219.7+0444?ï¨,°aa@P˜0O‹YÀ:Ÿ܉Ù2À<rœ…dž@ 0]E«Zâ?þÚÝð,M?Ä˒ûoÍm?½håq´MO?÷ÚÀZ΂¯@—ÎxèI¿ïI$i¢?ïü¿ÙŸC'¿Ð3VćÙÔ¿ß«Ø ër¿ã¨bõ˜ñ¿Îîï¡ãê÷AGNbllNVSS J121945+044621?ïýˆ–vj?@¨	¿¶•?7»LL­?@¨	¿¶°?ï÷"}Q'†?d|ƒê½?PÙ\ÚóÓ?d|ƒêº?ïÓ{–ãc?~G
BŽo?vB4þŽNI?~G
BŽq?ï&º-ßJ?‡]Ê980Ü?›<¨ºD¤?‡]Ê980Û4FGL J1219.9+6056¿ãJÂH õ@KãEŒÒ
úÀ:ìdoa'À<͒…©!Í@&ðڞ@VŽà3·?»{ÚÉðO¿´á%Ž?øeLöRØ@ãƒJLÕF?í4VCÙ¿è7…½Äœ'¿ëË!{û¤¿Á›!Äuæ6¿ß؜cÎ[˜¿ïÿõEq#AGNbcu3FGL J1220.3+605587GB 121716.0+611442?ïýXˆ-¯?2ÌJŒb	?5?3¾'•?2ÌJŒb?ïü¶×åµå?PJ̏ö'ð?:I@ÒPßë?PJ̏ö'å?ïÎà'~¼§?}9ežÕ‡?x·@¡¬å?}9ežÕ?ïéhŒ®g¢?WrŠ½1`?f—sQ˜^1?WrŠ½1r4FGL J1220.1+7105?äÉ#sM–@Fèdìé¢ÆÀ8¨Ê^]ƒiÀ;ñY¡\º@R'Ž7»@'a|ÚQ?£9hs³?ÀÃøzût@­'w>$ÿ@ Ú¨Ø{Ø¿Ìe{Yè~¯¿ß?YÐ,¿ãÒú
w·È¿ælfû·›ã¿éÍ•I¨À¿ê7@Iq8AGNfsrq3FGL J1220.2+7105S5 1217+71?ïµÝ÷×Ax?€GæƒË°í?'ˆ'
/¢O?€GæƒË°í?ïì\AàÇ?z¹ã%q'Œ?c£¾ä9¸?z¹ã%q'Š?ïvgüt'?'7Zÿ h?'?"qzÛ?'7Zÿ g?ïû¼Ml,?2Œ?Óv«¯?AÊOOï?2Œ?Óv«›4FGL J1220.1+3432?ï=™Ï'ÿ@T»ìª¸¦À9áéÃ}˜²À<pȖg"@°˜a¶(q@l÷¢cl·?´زP\?®¼œVÉw?ù³·‡Á*@	·nN<N?ï"ÊÀ9¿Ü…SÜ¡@¿âÓŠS«¿á¤…†"¿å>þ]hã¿á,1·20ÕAGNbll3FGL J1220.2+3434GB2 1217+348?ïüK'H?7ŒÙ7»–a?=¦Å¿ïï?7ŒÙ7»–4?ïù ïZN3?_fýOá‹f?I|B–Ç4ˆ?_fýOá‹]?ïãª)9z?x¿¦uX?lUÖƅìr?x¿¦uX?ï¦o~Õä6?s9új:Þ?†d J†ò"?s9új:Þ4FGL J1220.2-3713?æüA±œ¯é@9;·Ç'
1À:?ÐW›ÈHÀ<`«l)ôÆ@ ã(å?þT·Æ«K?ÀÖ3hb??¼,žïnã8?ý©ÙgåÂg?ûkcˆ»zë?ïûG¿1X¾¿àœÊr/ȿޔÒ?R{M¿Þ@)È¿ÜjÈéÕF¿è]'ømåAGNbcu3FGL J1220.1-37152MASS J12201982-3714137?ïñÈ,H ÷?Y°KÔ(¦N?\o§o¾e?Y°KÔ(¦G?îüi0ÔH¹?­lò'?? 9lò»tY?­lò'??ïÍŸÎ!?{AƒÒTy?yr°r˜ïd?{AƒÒT€?ë•YvzÛ?¢
ۓµ¥p?Áªš&¼"?¢
ۓµ¥p4FGL J1221.3+3010¿ß'ä¼už@T¯ke©¨À7ڊèü®<À;/jWWÖ@ Ó]<F,?ú£%"R? B³·[? ³~µßî@ƒy³J@a· D%¿âSÇÝúœ"¿Æ‹sü|ô¿ÜÁ¿àáW¿Ñ†±_ˆý¿Ý—|ˆçš®¿Ã[Â"¹=AGNbll3FGL J1221.3+3010PG 1218+304?ïýI‰Ó£ó?4º4»WÊ?5³±bàn"?4º4»W±?ïù÷O_:k?W"›î(r?H"ƒPÚ?W"›î(v?ïw¦‹ܛ?)p;¨C?'.ŸÄl¥?)p;¨C?ïØÍt=¿?jLó ?s™Eöa 9?jLó4FGL J1221.5+2814?éС@°Dý@TÒ//˜tÀ8%\±À;¶i©çÅw@ò®¸dµâ@A(¿<?—`°Þžu:?•š'Ç!?ú/<-­¸@çuXǗY¿Ý—m$E¯¿à¼J~Sm¿ãGüMÃØ2¿àvÚ݆®Z¿æþ\'ÑN¿â°–5a
ÝAGNbll3FGL J1221.4+2814W Comae?ïýà÷Õ?,U¥Ú¯%?0øCƒñXp?,U¥Ú¯?ïû~G¯rZ?Yuƒ^c»­?BáB6'ø?Yuƒ^c»Ÿ?ïÎ
㷅?°Úìço?xùs$=?°Úìçp?ïÿV;w‹?L¢¥ñ]À?8–i?L¢¥ñ]4FGL J1222.0-4121¿Â¹¤ûËÞ@5+ç:6\³À;R[LVñÀ<žË'±ñ@Û®Š—s$?þ鬆Ü'´?ع¶…Ä´?Ó¾-b8Ú<?ùÕt;;?@äïp¶Ç¿íjΪó^?îž8£NN¿â/0¤ãy·¿Ùzˆ|Ê=¿ìNOÿFǐ¿ïÃn_E°AGNbcuPKS 1219-411?ï°ƒ\7?ƒéˆõâY?ƒû(ør•?ƒéˆõâZ?ïîPcEÀ*?yÃG&á&É?a¯œº?Õb?yÃG&á&È?î,»GŽ€Ð?œõV©a?­4K‡òø?œõV©a?ïZRö²œÞ?'Z•¹Çê?"µ¡)¬d?'Z•¹Çêƒ4FGL J1222.5+0414¿áL²P•v@P…à`þG™À8©åÂg=À;ÁR4€:M@`5C-Ò @{íx:¤?ª	*\[0ä?¸ªê¤ÏÛ@¥åNë @R'{ÅÉ"¿Ù€	e.'õ¿å‰>7s3Ô¿ê$úö«Ãh¿ë©%þ—J¿î]¦Ùóü¼¿ïô[¼¿8AGNfsrq3FGL J1222.4+04144C +04.42?ïý…5[M?3ǓÂn<‰?3ÔU%?3ǓÂn<Ë?ïùHôµ?d÷Ö<Ïè?JÜ/Í+–Ø?d÷Ö<Ïî?ïwMçÊû?‰ä3ž²B"?'C œJ?‰ä3ž²BŽ?ïñCbIÕ¨?Qÿ))º?]y;lT°|?Qÿ))¾4FGL J1223.0+1100¿ì8W«áGU@R#ƒQX¸(À:èâ©­ãÓÀ<'Üo×ÿ0@çQÛiô?ü¢\¶º<?ϲ'´¤ã?̯ÀâÞ±ý?þæ"/•ð@8Ca©"7¿íœºëù¸¾?¯Þcß3½Ù¿çÖåŠ2ôI¿ÂÀbX¯o¿â¡¬ÃB	¿í"M!ÆÏ2AGNbcuSDSS J122307.24+110038.2?ïõÒÐÃü¯?R§'ösO\?TZ^x¢?R§'ösOQ?ïúWƒ`?bRo7ÍLû?F¡óŽ•¿?bRo7ÍLù?ï_h‹Ñr?†Ã|à'€6?‹è%Ý£U?†Ã|à'€;?ï§'÷Pq0?tp%¥&æ×?†6+ã´?tp%¥&æÙ4FGL J1223.3+1213?Òçsåë¬@Rm®ˆ*ÜÀ:Ü<I\jdÀ<d É8Ö@ãw¾RŒ@é§;BÌ-?Í]f"â?¸†›:…?à±¢z¾¸@ámÛhò¿È–œd$AÔ¿å"«=0¿êî±##·¿ÕO*u¿ï¦Òœðf/?íI'w"AGNbll3FGL J1223.2+1215MG1 J122332+1208?ïçûF?h:¤/ÔN?hï~á»?h:¤/ÔT?ïôŒŸR'?i¸vϵ=?VæÁZÛà;?i¸vϵ<?醙EwPa?€é	ҏ(	?…î¢+çŠ?€é	ҏ(	?ïÛ¸E?eW†ö£|?r#öÝpô.?eW†ö£|"4FGL J1223.5+0818?í
ÍÈ]€@Qƒ±mÀ:Å@ªÀ3À<Šéåˆ@ ׬NÓ?ý–:iˆYÖ?ÃЎã³F?·¨˜:	?õÕêî ¬@	nÀ
òwV¿ïû5•äs?ïÿ¢bô¿Ù·?œÎ€¿Û@G¿é=A^Å\?"ÄÃhõãAGNbll3FGL J1223.3+0818SDSS J122327.49+082030.4?ïþët‡ÐN?jPä£ó?!H·'û!†?jPä¤?ïü‡ƒÙ"0?O!N셱?;Ãá3f€×?O!N셻?ﱔý@õ?ƒ3ÃüYÆÑ?ƒšÀ¯ùƒ?ƒ3ÃüYÆÍ?ïçã{?_(‰­&`Õ?hô"ïçÍ?_(‰­&`ß4FGL J1223.6-3032?êä¸iH@?ò'B³÷À:Ìsí7¦_À<~ã¬bå@!âv"° š?ù"»¶úÓp?РS\žfˆ?¶çxŸ£ô¼?áqºøŽòw?üHÈK2ÙF?ïýœ"Šï]¿á¹ddIV¿í½÷|£¿?á[æ°£¡Z¿à-ä>ÙZ¿Ñ"î¬ñe3AGNbll3FGL J1223.3-3028NVSS J122337-303246?ïÿ]L þ?esÄ»þ?V{à.3]?esļ_?ïùÍ02'~?cÔ a…ð5?HË?7b}?cÔ a…ð/?ïÛÌÈpd?v—)/è.§?r›öGÎ?v—)/è.©?ï›ÊEö?qÈÚIËÆø?~²Ýÿb?qÈÚIËÆö4FGL J1223.8+4649¿¾'åÚ·¹@Qda¦
EcÀ;ŠRuÚÀ<í±jp·"@QP=/5x@Ç¢ PØ`?É|üÕÔ¿Õ>bŠ?³ÝÝ@bp¸@°"õ¦o?ÝCiv¼¿ç'Õ1\½¿ã§gž¿â1_œÈù¿âdµ—&¿ïýAt>–>AGNbllRX J1223.8+4651?ïõÜ°YŽC?L–»n?TFŸLãz¼?L–»mú?ïý.³:b*?T"lmR"·?6Šf,î±ú?T"lmR"´?ïåPqèٚ?tþ¡‹l ?j¯Ž&fÿ?tþ¡‹l­?ïðCQ&SÄ?I/ò‡Yû?_y]³Xx^?I/ò‡Z4FGL J1223.8+8039?̅ø…gºE@B2u¸eÀ9dFøâÕÀ<®=•ŒÅ@^.$*¬§@ð[|þX`?¯¤b ^.ß?ÀE™'7Ð@11eәp@
<Èý	€‡¿Ýe[#'+f¿Ý)Ucߣi¿ã£C_1¿âøû^°¿è9îlȿ캫ݓïaAGNbll3FGL J1222.7+8041S5 1221+80?ïf¥"­Õ?"îü1"Á?"+[¿JEY?"îü1"Á?ïrLD?©«FqQÑ2?'½¾–np?©«FqQÑ2?îWû§%Ë? s¡¡<ø?ªŽPE£M? s¡¡<÷?í:(j!Ê@?˜ã5¸_
?¶.¼®ñ®?˜ã5¸_4FGL J1223.9+7954?Õ˳Heµe@B''͖ À;Q,50"À<ãQN§-@!Ç&Š-jò?úâ_:øúR?Ζ[K«$?Â58†">?ñÇ7a–@Qõx'â?ïÊýê¦ý¿ëÒ§7E¿Ó"MA§?J¿Ø݂'™¿¹T÷S3-Õ¿éh¿§J\EAGNbll3FGL J1222.7+7952NVSS J122358+795329?ïþ¿Z¶?$9ëSÁ[?'úT¦4?$9ëSÁ«?ïý_rý3®?OýوI$?5hbŽä?OýوI'?ïð…Ázý?l(¡u[šn?^ô}
Ï.?l(¡u[šb?ïëß6ƀ]?TOoi)??d É9¤+?TOoi)?4FGL J1223.9+5000¿à€«6œWp@P¡]N°À9¯£¯À<:ʄóð'@³ªºG@YÀª›?³3Áù_'?ÌÁ³éüÞb@-nÎõ@þû¡v‡Ç¿Ì^ÕùFRu¿à4øÀEªÚ¿ç܃ÄE>οèçüÓû•7¿ìÙ@¿ïÿß´0ÕAGNfsrq3FGL J1224.5+4957SBS 1221+503?ïŽÈ‹Û?†òm…èE?ŒMÝ9ýÉ/?†òm…èE?ïòƒ%ƒ7Ç?m£,q2|?Zù´ùp=?m£,q2ƒ?íc©¢›¾?£ßÊ·þñE?´â²ë"Ð?£ßÊ·þñD?ï¹ÅƖô?m^«+–°?ŽºNZC?m^«+–®4FGL J1224.1+2239¿äiÛ‰Úþ@T—W'ŽžÀ;^ÆùN5À<¨§<‹Â@"p~]?ÿßCÇÕí?½Ð­¬ö¿"ãL@€?ýáçÌ,"Ý?ý%.»TTk?ë˜> N¿¿íA+®Ús~¿árߪJ¿æž©/"¿ÂúŒ¤¿ÙƒöduË^AGNbllTXS 1221+229?ï÷EäKǐ?P¤AêÞ?Qt7hpàH?P¤AêÏ?ï´çœ.§+?¤Ežœ¾?'ÆôV5—?¤Ežœ¾?ïµt¼¡"?"iÁ£'q?'¢ÿÐ×·i?"iÁ£'q?îYÎ6û5?¡B†p·"?ªcL®´?¡B†p·"4FGL J1224.4+2436?»­Ðù¸T@TÛÀ~à°¯À8ûDæ¹ÝÝÀ;æàyQûu@А'‰Úà?ýג"¬Ó2?¨³×]tzP?©²Ð]Œ3f@ç|¯Ý©@¾wä"?ª¡;¾5ôó?±qÚbâx[¿Þw†®‹¿ÜKêd7b¿ãŸ¥'(^¿ÐjiÀ¸íGAGNbll3FGL J1224.5+2436MS 1221.8+2452?ïýì?¶3.?&²Jb}?0žNf‹¶?&²Jb…?ïûXøûæº?YW÷G©?Bœe>?YW÷G¬?ïãs¢8®û?t|ºbþ³?lŒ]ÇQy?t|ºbþ­?ïþUž$K~? =zT°&@?*¦»H³? =zT°&ª4FGL J1224.7-8313?ì
•­ýÄÀ4e¿œb¡¶À9lʍWkøÀ;ü¢¥±ÕÑ@®¶â)Ö@Ø©_	zÓ?²¦_¿r
"?³¾õsµ'?ývqüœž1@
!+˜	K®?§]	pl#À¿æjW®Î¿çèGçöÿ¿éILÌKž¿åÓ´EíJ¿ïÿË&Ú_]AGNbcu3FGL J1224.6-8312PKS 1221-82?ïý•j¬a?2u"©Rëä?3Tªœ÷Ëu?2u"©Rë¢?ïöÌoÊz?ot³Æ_?Rg kt?ot³Æ`?ïÑ­'O?s¨"–v¾?wx©¾Ø[?s¨"–v»?ﱍ»V
?piíM	?ƒº\'*}?piíM4FGL J1224.9+2122¿ênåY@TjWÑx-8À6Y‹zՉÀ:üÎqèz¨@ã™%ÖS^@9{úLaØ?'<cï¤Ï>?§|€Úš@aS¢>ƒÉ@#؅c¬¢¶¿Ð[¬Cjbõ¿â{R¼ev|¿å¤«{Cm=¿å³@ߙ-¿çÒ(@æпäâÀ‰Èk>AGNFSRQ3FGL J1224.9+21224C +21.35?ïßbš°­Ý?¤‡ú"¨Z?pN²§©ð?¤‡ú"¨Z?ïé*ùd³Ä?èFómZ?fÕ›L;<?èFómZ?ïÁ&®B ?'X¶*‹Á?l¨òÞð´?'X¶*‹¿?ïÿõÈ"NÔ>Ñמzί>Ôo»bY†>ÑמzγÓ4FGL J1224.9+4334?àzµ×@R-gôÛߏÀ9çÁŸr ¯À<•ª¨µ–O@zýÕÙ:ï@kh¢×0?±ãˆP m?–œÇ nM?âF$!Gxe@ÁçAî
¿Ò1žBuÆ¿ä,4 ˜ü¼¿æ§‡-†K¿âÚ|îh(¿ë1Ûz¹×¿ïÿúŒ—ÓAGNbll3FGL J1224.6+4332B3 1222+438?ïaŽ¶l?¦Mz—1?"Î=i2|ó?¦Mz—1?臨¤f§? éNhA?†Vø&V]? éNh@?în`Œ¢€Á?š¬õn´¢ð?©÷5×óà?š¬õn´¢ð?î5@Ý?‡²"ø>?¬¯ò.?‡²"ø?4FGL J1225.0+0330¿âüj´'±@PcJ¡!À:Fþ»\bÀ;º2ƒàʱ@{õ&]6è@-{~%ŸÍ?Å>éõ§Œv?Ö,Ôz¿d@Q)`Kš2@×ͧS¿ÒÏß[š°p¿àìJ«õ¼°¿ßªT|ÙðL¿ê eêV ¿ë68Ág"ã¿ïûµ¸´AGNfsrq4C +03.23?ïUÆ	x»Ø?–üQ)¾ÿ?•G>Ðè"Ç?–üQ)¾ÿ?ïûP÷y#/?XìàUF?B¼"sG|?XìàUJ?é±Èß@]?®r`Y-¢?˕8܂þŒ?®r`Y-¢?ïý;ÔÒJ?*ZE=>?6'Ym³?*ZE<ì4FGL J1225.3-3446¿'ÉßθŠÐ@;Èä†&öÀ;;ª]6;üÀ<›ÅPä@ e;Ó÷Ž@òü¬Žhä?¸xƒÚ¿¬-£ <G?ìnƒÖ¹µ™?þ¨XÓÖ¬¿áo0«¼²¿åT[זT¿éjêŸpž#¿Öö†oj¿ÒfuÞÝq¿Ý""ܯAGNbcu3FGL J1225.4-34481RXS J122534.0-344737?ïõß'W[j?MýõŒ-?TA±QI/W?MýõŒ>?ïür'gS¯?Tp$J"7?<klÅb†1?Tp$J":?ïïËYæZ¼?fþ2YxžZ?`4¦¥D´?fþ2YxžY?ïße@ðx1?^å#¦'?pM_‡Ãç7?^å#¦†4FGL J1225.4-1550?·ÿïˆÞe@@GHf^ê–À;Á_0ϬÀ<ÔL~]Óñ@"8u¹•?óv ž9%?æT~!nÑ?á–
˜à66?ÿw¤as¸_@—|Hzî¿î¹6b<¶?íkawê?ΞŠŒ‹i?íêó((Š¿Ä õÙ`ƒù¿æåfâOAGNbcu1RXS J122525.2-155251?ïÔ9,Ëã?|ZT8vúu?uãiøšK?|ZT8vúx?ïûㆎ
?_àH¦ó?CÜqåÇ΍?_àH¦é?ï™ã:åª?†|aNö?‰‡8ñF•‡?†|aNû?ï÷*X3Ç?KÈçŸÝÎh?Q«Nå˜só?KÈçŸÝÎu4FGL J1225.5-2851?åðæÅr@@Õc¡ À:……žÙÀ<\>ª_º{@¾DVñÿ6@¢ÃÉîËû?ÎRÚ'C?ÕX"Ì@Ž-À,«Z@	OS;;jd?ï¨3PD¼¿ÚYÞb÷F¿âQ žÛøº¿ì˜Á‹¦¿ÙàÀI±¥¿ïüvÄ AGNbcuAT20G J122515-284956?ïÛ@
Ÿés?{%°Ž?r_ù0Eù?{%°Œ?ïû‡Û>¤?V¸4Êu?Cà"i·?V¸4Êr?í¿ûSsBa?¡ëÄwûÞ?²%deì÷?¡ëÄwûÞ?ï³æüی?qÕ!P³?ƒ{€Éë?qÕ!P°4FGL J1225.6-7313?ëHŽQ€À$é³ÃçÀ:0þæ$À<&A
çI@jђ"Q‰@0;7äs?½ÊÔÏû€i?§:{Ñ݂Ó?ïô&­é³@	JÊ©†ø?ïý•ø$il¿ÅÊEÞÜnÖ¿èÒ»YS¿×ª½®KØF¿äç¼Àæ¿ÜÞùÀJÞKAGNbcu3FGL J1225.7-7314PMN J1225-7313?ïþ+BH?00ú_IÞe?-N_‹Ûy?00ú_IÞ|?ïý
ˆÑâý?\gÚymG?7«¹pèŽ?\gÚymS?ï꽃¬Zy?ia;óÕòf?eB|S¥…Å?ia;óÕòT?ïç̒X&?TÇD– Õ0?h3mê§ØÅ?TÇD– Õ/4FGL J1226.0+5622¿Ô²1±;Æt@N4oÞµ,À;ªß<;À<ÉLÙÍfP@ÿñº—ëï@k¯–[ ¸?Åta¼2 ¼?iDúIÚ@JæýÐ?îÐó7š¡¿èá
¡~¿åáOp€›œ¿ãâ*⬲ü¿äÁt‹Z¿ïÑqÛÖUAGNbllSDSS J122602.81+562254.6?ïüÊÏÑu?5çSÊ}D?9©‡!tSó?5çSÊ}H?ïügtWz+?U/<1 ¯Þ?<Ä]D.®o?U/<1 ¯ã?ïésœäÑ#?g£xðŸ?fŒc.ÝI?g£xð?ïò"}Œú?KC.Ɓ#?Z÷æÜÝ?KC.Ɓ4FGL J1226.7+0637¿ïúXãYŸ@Q+OKD¢À:ƎyªæÉÀ<-†K<@!? &¼x?ùUɯáÚ?ÈG•*tÝ?Â[–ÿ‹eú?ý@|&©@Ç`QN|¿ïÿÿ&¦³?ïÿýç!é¿á3ÅP˜¿Ábº_aåM¿ÙVE'¿áYgŸ÷V¹AGNbll3FGL J1226.8+06381RXS J122645.2+063906?ïÿE¿E–"?T}^«vé?HM;Ë ?T}^«vü?ïü)àå!?VWÁÞ~Z~?>°ø×~ûJ?VWÁÞ~Z'?ïÛU
6D?wÛþÊ,¯¬?rrUzäÞ?wÛþÊ,¯¸?ïç°)r[=?YÚ.Áä-?hO֍¤Â°?YÚ.Áä34FGL J1226.8-1329?´²}V.t@Hxª*sÀ9‹}¼ÄÀ<¦†çæ.@LÒ*?þò]€
×?¸[ìÿŒ™?¾#әŎ@PŸ}i[@Š Õ¸"¿×y çÁÆ¿è7k§^¿ÈI?9%æo¿á€`"•¿ä¤&Eüd¿Ð7œ'"mAGNbll3FGL J1226.9-1329PMN J1226-1328?ïýN»½Ø?33¤ø/'?7½Š"<Q?33¤ø/€?ïúÛ÷óPŠ?X'_ȱ»t?D 2½Ü(?X'_ȱ»[?ïß´—EL?uZ¹Õíöå?p%´tÝZ¶?uZ¹ÕíöÛ?ïæIP…ÿø?UˆAÓ°?i¶¯z	B?UˆAÓ¸4FGL J1227.1-4437¿ïð–Pð—@2­}|,¡À;,‰ËÆ=À<šé+¨$w@!8 ¦n?üËyæuë?Ìc¶ˆ½©C?¶dt^Kº¿?흨;ic@ºì*
?Ÿ¿å­4¡Gbë?ï©3g#{¿êŒ5-w?Ö©aãŸÍ¿ãÈÊœ£¿¿r¬šÓ+AGNbllPKS 1224-443?ïÿBâ%Ý4?ïSõ.æ-?£»DYŠ?ïSõ.å¬?ïù±ì:@?o;ãGQÓ?I8Oÿ¬?o;ãGQÒ?ï䚩X=Ë?q&&bz"G?keV§Â5?q&&bz"T?ïú9‹ó^?>CQ}À&Ž?G‡Ð2ƒ)?>CQ}À&U4FGL J1228.3+7521?æǧãÿPÑ@DØ	þ†ƒ<À;XèQ'NÀ<ý
)N­ã@<…—Y"†@è1AÁkp?ÑPÂœÇÌ?®Ùx_jÒ9?×w*#?P?ÿÀwÜÛb½?ïò…ÞѲ¿äʬ+l•U¿ÏõUҚl¿ås`'¿æ÷œ"/¥	¿¾[WáAGNbcuWN B1225.8+7537?ïû©Ž7?@¤Ž§6p?AYÉÇ"©?@¤Ž§6h?ïûìÅÆà?[‰p7 f?CäLè䉈?[‰p7 i?ï¿ntæ?€EÛP`æ?€$bÆx?í?€EÛP`æ?ï¯t#eÙÊ?pEKw?""÷&‰5?pEKw4FGL J1228.7+4858?å;uxnî@PíTK±¯:À9òÈlüÀ<PhÍK@áîÇôK@xéö©??»vapD?ÁA;ß,@ª#9Àëî@Þ<)Ñàˆ?ﲋ£6ÑM¿æ|zo1ç¿æÕ*Ÿû ¿ì%yÁâãå¿Ýì%!øxL¿ïÿjÿR[AGNfsrq3FGL J1228.7+4857TXS 1226+492?ïü=ÎLÛ?@}á'Kl?>™'øÙ?@}á'K€?ïü'e|Á0?PCkáۅ?;lÔöŒ!?PCkáۉ?ï›Gw²&#?…o™åäJo?‰."vwv?…o™åäJv?ïò¦Jóµ?J
¶50?Z³j•ÊR?J
¶54FGL J1228.7-0318¿î¡âV´@Mˆã£¨çÀ:`*yPMöÀ<YÊ1çٙ@ê¢îþG@¦^ÛX?Á6šÜ9Ò4?±áàZHJò?ðþ ŸGX"@}Ðãe–¿ä¬ýpÇ?îÙE¶Ãv¿ãñ6É>£¿àTÞ긿åÏó'ªhõ¿íþë}'üAGNbcu3FGL J1228.4-0317NVSS J122900-031758?ïø¡ã@ö?KÑÈbc?^?Mxsžü"H?KÑÈbc?W?ïú‡Õ$+?^šyP¼È?Gõà«oTd?^šyP¼Ö?ïáLù]?s"¿
3$?nà³¢ú{?s"¿
3?ï À4—,?xè?ÑþÆ?‡ÏòÚ>´ç?xè?ÑþÄ4FGL J1229.0+0202?ãÊkk‹/@PwpyåŸÀ6ä^}cØíÀ;HŽyªæÉ@賖ðÇÔ@ë5ó×ӑ?Š Îc*À?¸µmŠœü{@"›y·|°@!¸j¢Ž5¿Ø®gÜÞï¿æ#
%󯐿éêPkR^¿ê‹*k
•¿ëó[ÂHf¿ëŠ
_ÕR­AGNFSRQ3FGL J1229.1+02023C 273?ïñª@öèc?_‹RT³;?\«~/:)?_‹RT³7?ïãV=#_?'ýI-µ?l©ÂÜ áq?'ýI-µ
?î'Û7Íä¢?¡
®´òó?§ÒLƒ!µÓ?¡
®´òó?ïûg;ötý?9Ԕ¬À$?Bc&,	O?9Ԕ¬À)4FGL J1229.7-5304¿Ø0˜Ÿ˜ðà@#SA|¢À:lT¼ð·À<3uÇ,z@/äbÀ"…@úb>¹y3?·¥ÃH"™U?pN¦þYŒ?»breù7@	2tÔ¾2Ö¿Û¹4i"P¿Ø»b¿ã6쐷rÈ¿ãºI!²o¿Õ;à^d¿çú
­g¬¸AGNbll3FGL J1229.8-5305AT20G J122939-530332?ï÷Q8t¸?Kï·½':?Q]öŽ€?Kï·½'?ïüë°{X6?`ÉD•=ï?8¢|%>N?`ÉD•=ï?ïç¸Äo²?n
fI`!?hîG;N.?n
fI`?ïü7Ì
ÖÓ?.ª'¸W|«?>AŸ'Ib‰?.ª'¸W}4FGL J1230.2+2517?îb/®‡L8@U9ý6÷ãÒÀ8C-|:
À;pb·…<ë@Ë[HÐÿ7@ÝBeÖ?›±Ò vX?«Òƒšÿ 4@t/øì@ÓÐÜ{ì`¿Ì8¡1=®¿à‡ÂÀð¿áW_,¶Ap¿àãeË5óØ¿ä+4+€·K¿èjÜí¬@AGNbll3FGL J1230.3+2519ON 246?ïþµ^fœ™?Ž] 9žG?$ª–6p?Ž] 9žS?ïùà†?X\³!nTÆ?Hë¡çí?X\³!nTÉ?ïՂØDŸ8?€3	œQ8ü?u>"Ý°bù?€3	œQ8ù?ïÿíëÒh8>ØûäµàЫ>â-—È;>ØûäµàÖö4FGL J1230.8+1223?ßMçÍ[=@RŸag#$ÈÀ8ÎIÚ>¥À;ân×N0@o&ëÒ Ÿ@5Ê¢P!?¤¾ÿô[K?¡íœƒ·b¶?ü84ú³@	=¿©"Ï¿Üj°¢õá¿Ø†3çüÔ¿ãBU&
±¿Þó·‡Á*¿æg;¾G"ÿ¿Ð6äΊAGNrdg3FGL J1230.9+1224M 87?ïø9Ðy´?IVåE?O¾.V?IVå<?ïõâ#ÆcA?lðùAâeã?T;¸s9í?lðùAâeæ?ïÔÔì6ô?÷u. 0ï?u•‰ä…õ>?÷u. 0â?ïi.ˆt?'™HK­¹9?'Ú?nÿQ?'™HK­¹94FGL J1230.9+3711?íw*Ð+#i@SÃXdE#öÀ;kGï'Ú:À<¥}I׺g@:P$/µ$@"¿Z'È?Åáe¶K1¿³J²«¹VÎ?îÓë¤ÿ(j@‡/.kÎ/¿ÑÓ%•|)¿êµ
(¯G¿îÕâ Â?މº¾ØBw¿ïÿèÅPØ¿éièÑæAGNbllWISE J123124.08+371102.2?ïôîmÖ¥?V%$F¯?V#$SüµÆ?V%$F¾?ï÷®â4ÀŽ?lQîxz[¦?P¢;–~ã\?lQîxz[¨?ïÀ2oŪn?-£iPÁØ?æÈ*ÈÒ?-£iPÁÛ?ïé"äDp?eíea^»¿?f{ð»5?eíea^»»4FGL J1231.5+1421?搸®ùG@SÀY!À:YoÒòåÀ<]|Ìy1@ ©.§ˆD³?þ8RÆvq?¼é}1®ù¨¿vª­Nh?½Yۓ"@°ÊnΔÎ?ïڋ1!
<¿èŸݵR]¿ä7sŸ4
N¿Ó¢yg¿ár6é¡꿳ÆóDç›AGNbll3FGL J1231.8+1421GB6 J1231+1421?ïþ'DáS?$]ÇAmã²?.m‹±ê¿Ž?$]ÇAmãr?ïý/¥[T´?P~ðFö3?6'Õ%ZOã?P~ðFö8?ïø1ƒÙ?co*'ü?O;ý󬖭?co*'ü€?ïã8Ýd•?Zø­lE"?lÇ"ý›je?Zø­lE‰4FGL J1231.6+6415?åÀ"šPÒE@J^j¹¦À:"k†`×±À<µ+úYÍÒ@ 0@ºÛ2Á?þƒ†'e n?·8Ô²ÊB.?)˜£i—ïY@sVOiu?ß^ќ•Lƒ¿Úª¶AÅó¿ã²¡r«ï¿Óù5@S­&¿ájQýù•ƒ¿ÄÁK#êÀÔAGNbll3FGL J1231.5+6414MS 1229.2+6430?ïöŠ"s¾?JÝç«·Ì?Rê×Ї?JÝç«·×?ïüd©Fº(?TšZW¯æò?<ÚµÊ.Âß?TšZW¯ç?ïì€PpÑ?n܋o,?c€¯.ð?n܋o!?ï×~£¼r[?_Y3e"ô@?t@®!Æ҃?_Y3e"ôM4FGL J1231.7+2847¿æ×1jRøÉ@UUüã
®À8—|¼êºÀ;ÒÚý87@^ܯC?ÿFVüfŒ?¡šØÞÓàg?¤:à"BM
@	Dzãí@Û°ºG?ï÷ü@WÞä¿Þi"nå¿àWësÿߏÆ­°}¿à6YSXm¿åRÓº}AGNbll3FGL J1231.7+2847B2 1229+29?ïþ_¼ÿV?$"zÀé?*´0
šº?$"zÀ>?ïû¢›º>?\Q®Þ¶u_?Cu'O?\Q®Þ¶uV?ïà;)"€µ?v'·Ð߆ƒ?oÄÖlJŸ?v'·Ð߆ƒ?ïþz7?Ç?#'Œ'?(WŒ™]?#'Œd4FGL J1232.5+4821?íøzì0!@Qm3	AÈÀ:%…—"¤À<†Ó«.í@Xûu·P@_ND0±?¸½gÔûox?³^óUw«³?ø¯²$ªÚ4@m™È"'?²PúŠet¿âÜb¡µÇοãø™]3¸¿çž<á²·ù¿ÜæÿŸ¿ïÿó v,­AGNfsrqGB 1230+486?ïéùÒ#ئ?oÌ?V"?f-Ü'YP?oÌ?V"?ïõÛ îà?k€ù9¬ð?UðH¾"?$?k€ù9¬ï?ï»Ú  t?€ÒzîÚ|U?	W×âún?€ÒzîÚ|[?ï)äWY©g?†¬ý]??šÃuÊÓ?†¬ý]@4FGL J1232.5-3720¿î<¥e .0@9`ð¸,,À:'…€ÞÀ<M57ð1V@ Ӏñ5?þräùê<?·Óó?"ª—e.Ok?à3
^RÆ¡@ntÊ­7Ü?Òa¤W׿εœ¯x©¿àä/¿á,¿à)ᕱ¿ÉçΰқC¿å_iòâáAGNbcu3FGL J1232.5-3720NVSS J123235-372051?ïö/±ToÁ?S³ôK–?S W V?S³ôKŒ?ïý*ƒ`£?R!g²ÃWÁ?3~«äúà›?R!g²ÃWÃ?ïäÌ¥?uYán¼È"?kùè3í\"?uYán¼È–?ïð¿K5Ð?LOþh´‡?^i"_õF?LOþh´z4FGL J1233.1+1703¿íN¾;0†@SÄÝ?á—_À:ûÒvYùÀ< C~ÚÑr@ +ßâSG?öm9ôîT?Öç=¼N${?âX¼$@kªÃˆê@È]Rkˆ¿î™‹âvØ$?ïþT>p©
¿Ý¢¼'ý¡¿Ëvh›ŸÙ¿æä:ýöe¿ðAGNbllRX J1233.0+1701?ïø»(*<?JŠ8uŽ¯"?M_Wç
<?JŠ8uŽ¯4?ïóÝha?vì]þ•ç?XEó/=Çø?vì]þ•ã?ï5Ç91?'Ÿ-sÉ?™]§ßùé?'Ÿ-sÉ?Yš?–' ­U"?¦E/f_?–' ­U"4FGL J1233.6+5027¿ÖâD·=@P›'ÿÀ:¼pøŸöÀ<¨~–ÞÔ6@€ïW¼)'@ÑyÚ·q?ÄÈñ¶f.?Ä·©º,?ýˆ¨°Ò@³§<ðK?ï¿ÜŽá¯³¿Ý#¶]ÞØ¿çJ¶!œÁ¿ç´Uý¸}
¿è,œ2¿ïÿÿ)@k*AGNbllTXS 1231+507?Õ?¥¡Èr33®?£–ß•r®?¥¡Èr33¬?ï JL,?–ÉyeŸšs?‡ílÜ8´°?–ÉyeŸšs?íʔÛå0?£{ó˜^jƒ?±«Y ×æw?£{ó˜^j"?ìø69Ú7?¤‡Gñ=.©?¿ >N1.<?¤‡Gñ=.©4FGL J1233.7-0144?·‹É#
,n@Nhj¹¦À9@'üí&	À<ð'Íó@ðGÙÞX:@a̾Šë?«'Ìx"n?‰ÇcEj\?ÝG¡Ÿw@
î /àÃO¿âù&Çë¿ä,ggfN¿àÊ1|yÎ"¿àî…ÿ³ÔÙ¿àÚßI§ÿ¿ß§†¡ð*JAGNbll3FGL J1233.7-0145NVSS J123341-014426?ïûôÜÌ(7?6qײÝr?@,ŒÏ_'?6qײÝ?ïüòLnO}?LoNKÐs?8mœ"p?LoNKÐb?ïôǹhb·?`Bm62åó?Vp/:"Ã?`Bm62åú?ïöýcФÅ?Bœzïýá&?R8^¶u¸?Bœzïýá4FGL J1234.0-5735?ámúXK½@É°$öYŽÀ9 ø«wèoÀ;¡Ç¯VšA@jª›6Ó?ý1úNX?³…	>Ã	U?Àú¤ÌR©@œZz@	…™0=4"¿ïùw»"€^?ïâY'kÍ®¿ÕpB½ê±º¿Ýa%^ß3'¿Þèê8v¿å=»ýœ£dAGNbcu3FGL J1233.9-5736AT20G J123407-573552?ïó b )?\&±-Ë?Y¿;¿Á­–?\&±-·?ïT()ÐÔ?®C°HW–Ë?•zúÅü¥Í?®C°HW–Ë?ï6·
ä(®?":É¿–0?™)CzêI?":É¿–+?îK,¶½?–àpÇz	Ñ?®ËM4"/?–àpÇz	Ñ4FGL J1234.7-0434?îü ÷àóÒ@MWS£ìÀ:ó¥S?ÏÀ<}ÊÞ)@ 9훤`È@|ˆGä?²——`Ú¿Šu¨Î•Ï¶?ÈXŒÞö#@ϗ‰!S?àHLŸëÃ2¿×õp¥.£,¿ãæ~¤ ´¿åy0}¡@'¿Èüªµöœ¿ÞŽ{·AGNbcu3FGL J1234.7-0437NVSS J123444-043623?ïúÓVÚ"æ?COG<óïv?D²¤—tg‰?COG<óï?ïýc
¥?O(¬ªuDò?4çï'× N?O(¬ªuDû?ïägZ+A1?r*‡ð†7?k˜¥Ô¾Ïµ?r*‡ð†9?ï÷çÚÌèÉ??ëõ³v^?P0Jf.nà??ëõ³vH4FGL J1236.3+3858?ÈúøaÅØx@SoŽ`€sÀ:Ç{ÿTßUÀ<¶=Y&âÃ@íçÈ%É@`¡F6E?½Ša~†Sþ¿¥ ÿ‡?é؋Fð@/UÌ¿îîεY+?ÑW:Ä¢ú¿âé³ÊG¿ÞâʚÃeE¿Ûä×E Æt¿Ð5ÂY¬CÀAGNbll3FGL J1236.6+3901RX J1236.4+3859?ïû#ê؈¤?F8AõÆ?CpTÝt‰?F8AõÁ?ïýGkMC?NDÖ"Æ?5Ä¥—î#?NDÖ"Åû?ïñÊÈòQp?m 4l§€?\jn] ?m 4l§‹?ïïh¦Ç²?P{kYˆj?`—Y8îL²?P{kYˆh4FGL J1236.9-7232?ï¦i'•RÀ#bÀh ÓÀ:~¸–ž=À< ÕÓËò@3òA{ul@Øâý¹÷?È=~æ»?ÂØgµ›Ø¹?ý‡†Œv›h?üy6ð'®?ïÿ–¹‰$¿ç=¾Q‰à¿çw!r–u¿â=n€¿çç]<9A¿ïÿQ÷GËAGNrdgPKS 1234-723?ïÌs(ꦍ?I¾€E¥?yÆkŠ¬¹~?I¾€E¡?íjl=l1?½ëú¯óז?´¬žžw?½ëú¯óו?îtˆ	6ó?žÞ"ú;«f?¨·oìË?žÞ"ú;«d?è©° ú?¬¯‡šE•d?ÏÁY?›|?¬¯‡šE•c4FGL J1237.0+3019¿îfµª}š@U`‡~äâmÀ;Ú¶\GÿsÀ<ëCòž@#<Ï8ŒäT?Ѭû¡ ¢?ä9ÓÀÝ?ïÿÐß´0@Œ•¥RÝ?ùl@ûÉ?ïÙÓ`dĦ¿ï;üR?íÐÇÎ`Jÿïì%W¨]'?ïæÑÆ0ÑY¿à¥è'%1AGNbllRX J1237.0+3020?ïà&˜PTÚ?®7]Ee?oÙg¯«&D?®7]Ee?ïæ#òçto?Ž¾"¨-€?iÜ
‹'â?Ž¾"¨-?ìâ^_z]?£–U®Úª?¸í
$-?£–U®Úª?ïe[¦Ìü?áí—å?k?"T‹>f`W?áí—å?k4FGL J1237.8+6256?ïÞf"ayÊ@KåâGˆUÀ;¢Qó蚉À=
]Qï@!Ã1Ãq"?ÿ#¶¾mŽ?ÊZˆâ'0𿧓¡2OB?Ùxœÿ§€@A#ݪÀˆ¿ÞGAÝðá¿èðk¢æIv¿æñ?Þ<`Ù¿Ïøö¡]¿Ø´^a4Me¿ÝùÚ·qõAGNbll3FGL J1237.9+62581H 1241+626?ïÿ£×IÆ-?#ªH&å?
-Žt§1?#ªH&g?ïý€eö*?K|§´	?3ü×PN­â?K|§´
?ïø"'p?hÖR
 Ì?Owéº?ÔT?hÖR
 Ö?ïýí-ä¥?"x¹û$Õ&?0–"€ÚÉ/?"x¹û$Ôõ4FGL J1238.1-4541?Ýÿ9Š,@\@1df±æÀ:¡•ç]rÀ<MI)>¾@â
?#@*k
•?¹ÞÂÿª«Ì?µ b‹l?ùú>¥W<þ@"Ô§äá¿íÝ.^¸<?Êk|»<'¿ã€.Ä8©•¿âÆ®¥šXÜ¿à߸aÛ½+¿ïþE`zîAGNbll3FGL J1238.3-4543PMN J1238-4541?ïú,–©0?IUêhPyÁ?GM§Á[=/?IUêhPyÍ?ïúÿ)fD…?^#a߇?DZfíçÅ?^#a߆õ?ïÊ;"Àã?{‹v|y™?zýb5ŸŽË?{‹v|yš?ïì°œ\?QðSEG²?cOäcô£"?QðSEGÆ4FGL J1238.3-1959¿î–'N­Ø@Eb´·,Q˜À9¨ÔÈCÑÀ<>÷ÂCÜÏ@BÙ¿¤p7@Ǟà*w£?³j·?-"´?­FæÄD½õ?øcì8¢Þ½@
JGB‰½Y¿½:ÙoÈdÞ¿à`ö…,û¿á݇?Nõ\¿á­%!ͅ.¿êöM½øô?¹ðCŸgAGNbll3FGL J1238.2-1958PMN J1238-1959?ïôpvv‹?R=½¬)?Wçíç?R=½¬)ý?ïû"'ñ¦Q?TØꘫö?A­ô9f½2?TØꘫð?ïLî,ž?'»ÐKðž¯?–b=úlL?'»ÐKðž°?ïñ\bËè?MZŨ{ÐA?]ýG:h,?MZŨ{Ð[4FGL J1238.5-1201¿ëÈÓ¥<3b@I[ë[-M@À9{[ùûÚÀ<&=:óñÕ@	T¦ h@@휻	h?³c%ên?°oÁÙԝ&?õ1\#…@µòοT¿ØOãÖԎ¿äþ§°³'¿çõ²JÃÉ¿é2µßËW,¿îAy¢XZ	¿ïÿí )k3AGNfsrq3FGL J1239.1-1158TXS 1235-117?ïÿ¡;,;?ßYš.ð?Kؚx«1?ßYš/u?ïýk¤Å¶?J‹ú®¥å&?4§jÙÒH˜?J‹ú®¥å"?ïâ
ÄGƒ?iYôT­MŽ?mò;¸|è¿?iYôT­M?ïýÝKѧ?'UÕ|ì?1§rÂ&?'UÕ|ëø4FGL J1239.4+0728?ÙÏwf"kÙ@QˆÕ¥¹bÀ:;q¿_üÀÀ<lTdÏ@;݂|œ‰@èÿI Û?ÁfbàtõJ?¿˜á7èύ?öIãxà¼@%U-¥?ïù+
ÊÄ¿ÑÅJâÒG¶¿Ýò
ƒÌ'á¿æŠ=²èö¿çs[wN¿ÐÞÒn¥ÐAGNbll3FGL J1239.4+0727PKS 1236+077?ïÅÑ"Ñ?€Z´ÞhÄ?}ûî˜?€Z´ÞhÂ?ïïD©œ"?t´e؇®?`å»VckD?t´e؇®Ž?ïSîb?Œ¡åW(?•œŸ="¼?Œ¡åW)?î©àôw´?ŽC¿¡‰¦?¥a𸄿?ŽC¿¡‰¦4FGL J1239.5+0443?ïǚ‡R+@PÚôðØDÐÀ7†¸
"'rÀ;q'¬?Ž‹@àðfÚÕy@Ò¢§_U?—ê&yçL«?¿–ˆÌAâ@%|Q£"î@­ï"ã?Ð>ý'¿ázÌ_¶Á¿å%)œ±|¿æŠ ˆK>¿ì«»Û
p¿ðAGNfsrq3FGL J1239.5+0443MG1 J123931+0443?ïâ
Úqµ?wÊ"jöñe?mõá%ŽMy?wÊ"jöñe?ïÁl¶ŠÇ?¡Š
ë Û?I¤ºœuÊ?¡Š
ë Ú?íþQ3êY?¢ÑлàIh?°]v`­6?¢ÑлàIh?ïz×£ÙSý?"t†2_¦?¥"Õ€N?"t†2_§4FGL J1240.1-6846?îjÓ§W²FÀ²-"wú
À9à§7EÀ;çÇc×?í@ËÁPAáÍ@—Yûô؅?½Ñ¾¿?¶ÙþŸ¾ÝÝ?úCŠc›°Ë@ʯ‰ˆ¿à2Æü©3k¿Ý95@S­&¿æj]¡›Æ›¿âˆ?)5®¿äEœAi¬Â¿ïûC"¦%AGNbcuPKS 1236-684?ï¨!$£?'§Î@<›²?…÷¼6×??'§Î@<›³?﯁"!¼?•t5â·³0?"·w¾Q?•t5â·³/?îACß±?œ£æ«1Æ|?§+ëÂïV?œ£æ«1Æx?îERm£?"KàôaúÅ?«®JÙ%Î`?"KàôaúÄ4FGL J1240.4-2606¿ÅkPGŸ£c@BXc{ÐZ÷À:Ž£n.²À<;/•Y@€žBöŸ¯@¾¥<e?ÑFÆÞOâ?ÐÍž§ö?ûióžÈ­ƒ@¤­Q'Ñ?îê£aï^G¿æFGhÊ¿à×è‰ÁµB¿ßöÉàß(o¿ïÿùµc#¼¿ätü–¾óÆAGNbcuPMN J1240-2608?îxKIØå·?§±ï'º%â?¨{Kbq¤z?§±ï'º%â?ï¨dқõN?•U´ùêä?…æËY¬•?•U´ùêä?ë.:MX¶p?«þS¨!ïo?ÃGʝ&G?«þS¨!ïo?줐ZÉy?œÞYÅq…?ºÛE)´.?œÞYÅq…4FGL J1240.4-7148?ì~/©ÌÀ!ì´®ÈÕÇÀ9y=07FÀ<¤—ú])@ µß5°)?ýì
Š,>L?²'s°Pë*?—¥bzž¶?鍎]ü4™?ýÊâlFOE?ïö¯¿uÌ5?ì|c}ÓÀ\¿åÇ´_¾¿ÖÚ"zx—¿ÔŸ
â@ÒX¿äʤ~z|AGNbcu3FGL J1240.3-71492MASS J12402118-7148578?ïæÞõ.™?eaGo^?i!
Ñïeñ?eaGo^?ï{ñþ[µÊ?¨«lcï?À4‰F¿?¨«lcï?ü5ì?ƒXôk?‡'@ò»Û?ƒXôp?íÃÎ?§ˆÿÃn?·÷Ùäa'?§ˆÿÃm4FGL J1241.3+4236¿à…ÏƦûÌ@R˜Äq´xBÀ;²íþu¼À<¸M_.cÁ@ƒÔª;Ó@@Q8¢ý%?Åø\]#¹?Æ´¯Êˆ?Ï"jãù#?ü·»á2?Ó¤ —@¿ØÌÅ@'¿ê¸ÅCk›¿ïùϚ¦ã?ïÆìž#l¿ïÿþBe«+AGNbcuB3 1239+429?ï÷ §g"?\åg²ˆ°"?P¾±1ɽ?\åg²ˆ°"?ïü¯sJ]ð?V‹-	eØ?:"e­ð?V‹-	eÜ?îÙªSa­O?•ª¡VÕ#?¢eZÉå*û?•ª¡VÕ!?ïö0mÊf?S!a•M?SŸ%òk6™?S!a•M4FGL J1241.5+3439?ïÀ}œ•2@TŒ
Ã7!ÕÀ;'ë£Q©@À<¼tªÌÈ@ ŠõíØ?ÿ5۞÷§l?Äöš;*""¿—»£К?Ԕy^»¢-@|Bÿ*Ø¿ï´4_®t?î©ýýÇA¿åwø_!·¿ÄæËümNb¿ç†´ð75 ¿¿•°ÖÍÏAGNbllRX J1241.6+3440?ïÿ¨çÕ²?5äÉa/p?ÊãIÜÊ?5äÉa.Œ?ïýGl'С?LˆsµbÖ?5ěqz÷Ê?Lˆsµbã?ïëâ
Õ5?kWo ¶?d€õ*Ëí?kWo Ä?ïñbJ/?RïNhô?\å;Ýk å?RïNhô4FGL J1241.8-1456¿á	tۇÛD@GïAcwžÀ:$ÝpˆÿÀ<D¨ª®•@ 2J*°°?û3	wx¢?Á#øÙÉà?Æpè géô@8Œ{£åM@då²ÌÆ?ïï›2öÍ¿åhrû?»"íe»þ¿Óc҂™Lî¿çÏ÷Å¶¿Å	ä˜ AGNbll3FGL J1241.6-1456RX J1241.8-1455?ïÑ‹k'f?vßùŒj­F?wpºJ7M€?vßùŒj­H?ïïš!`Ó?s§Ã^ª?`eÞüŸ-1?s§Ã^­?ï=,X=Dˆ?'D_e¥?˜ZtøWnØ?'D_e¦?î^Dœ¦¶?'®"ÂUÆì?ª·æ5"§?'®"ÂUÆì4FGL J1241.9+0636?âû­VÃ@QV'è},|À;]Å~ú±âÀ<¹4@€@!#AúÌ9?ÖcÜþô_?âÞJ¹a¶?ïÿwTV™@KƧïž@'™Hæά¿îáóFí$¿à.ŠÂfA}¿ê8¨½ùË3?¬!
ä­š¿Ú'¾1(—¿ðAGNbll3FGL J1241.9+06391ES 1239+069?ïø…œ®é7?Rš ]˜?MéD[Í?Rš ]—?ïûq¡RæÌ?W蓰"[?B9z´dÓi?W蓰"^?ï[Šá4¤?·xÁWÕ?"Ž¾ƒÙkƒ?·xÁWÍ?ïïû§ ?a·l£rpM?`€Xùßµ?a·l£rpM4FGL J1242.4-2948?áˆv¬Jvu@@'-VÀ:ˆ<Ž%ÈÀ<7Cÿ3Qf@ìGÅ•Ï@@OÁß?ÐUŸÚ%zä?Ë9{â#¡?÷	f±@±¨‡s&¿ÀŸRK–¬¿èX;•ØCù¿ëukò—a±¿ïü"J|ûÔ¿ïªH]¼ÉŸ?§c¨¾GhAGNfsrqPKS 1240-294?ï¼Iû>ªk?‰´•Vfâ?€í0Ue\?‰´•Vfã?îÈ ò_mT?°}©÷‹[?£uðÚ	*Å?°}©÷‹[?ëÍFÞ¹ÌE?­‡jJB	]?ÀÊä…Îæ?­‡jJB	[?î})	a²?"d,=Øn"?¨-oiäÚ?"d,=Øn"4FGL J1242.6+7635¿Þ6‰Åg@DCÿÞr¿À<ºSM"îÀ=2ŠÙã5Å@"o»'!­Ð?ú%kå+hd?Љ
uZ ?­öœ)øæ?ၽí@?ýɸl«¿¤· YfÏ?çïMËdíÀ?Ñö?âÄý¿æÅ!²­<¿ÝÙôhI?ÒÅ0"åˆAGNbll1RXS J124231.4+763419?ïù·Ó—?IåmÄnÃG?IÁÉ ±¡À?IåmÄnÃI?ïø뿨³Ø?k9hö‹ï?LQ]0Ÿ­?k9hö‹ï?ï°\í»uÆ?ƒÕ0ûd?ƒèđ"Ž€?ƒÕ0ûd	?ï¬
Ë5"a?vüJ0àÎ?"ü2žçá?vüJ0àÏ4FGL J1242.9+7315¿Óïè
°F¾@Eí?)
»EÀ;.W˜mI¯À<ò],+6@ "q!€XU?ÿ¾ü)±ª? ªõ>¿£ð<àÓa^?às–V;@<¿á¬Ø¼?ïòÒO̲¿éÆ	>˜7¿ÐõDz®Fû¿ÖJªH=†s¿ä6¼ÿŸˆ¿Ï¥~ª*
–AGNbcuS5 1241+73?ïý¬lIa?.ZŠ×s!J?2Ÿ\´ì¨?.ZŠ×s!;?ïü›(*›6?SëϹ çö?;&¾«&]'?SëϹ è?ïö4REX?`òu®ñ•?Rý—[uOp?`òu®ñ‡?ïÒ?—Ô±U?^s+e¥?và4§U?^s+e¥4FGL J1243.0+3950¿Ç+dÔ4K
@SKGyBÀ:ÓG:Q5À<–jùs@ûrC>n@ÍÓB1Ó¸?¿‡î`ñ1†?s—'ÝR8?±böð6ß:@tà*?ë—­µ°¿æ´:æ…Û¿é=Ú rfO¿è:ÑÂÕÓ¿ð?ïÿþó…õAGNbcuSDSS J124318.91+395117.7?ïí/¤ÿL?föÈ'>?bÐ[ñ³)?föÈ'F?ïÝý­þo¡?"ßVp6RA?q)È/k?"ßVp6R@?ï¡Ë0³å?'êv/î!?‡3Ó¾î?'êv/î?ï²$Ž¹ ?{ô¿Hpx@?ƒvÜQ»x@?{ô¿HpxA4FGL J1243.2+3627?à¦hÓm­@T œ^o÷àÀ8d çk´"À;w²Ý7~@¸Á¾Ñ·m?úa
 ë2?£k/MöX?®#ÃöÝ@àj¾º»R@oÑ^¬Þ›?ï>S¯­'¿Ô^ßY—K¿Ùß͚ýòµ¿Ñeœ\AŸ]¿Þ"Þð¿ÛWQ`ñAGNbll3FGL J1243.1+3627Ton 116?ïÇøAÛ¢?w€?RýÖÃ?|ß.÷Ú?w€?RýÖÆ?îXà]BÀ"?ÁdÐ'ƒJ>?ªqú+ÓöÔ?ÁdÐ'ƒJ??ÕM%k?Ÿw"÷
åÇ?¦§Â«-©J?Ÿw"÷
åÅ?蟝.mþ?±h0,Íl?̓•‹FH?±h0,Íl4FGL J1243.9-0218¿éðӒùL@NA	Ö¶[À:C(0 ±¼À<f/çCq@ðÒ]…l;@]°µ??Äv¹Å³þË?ǎ_ê o·@w¥ôïp@au¼o²j¿Ý<û ŸÈ¿çËÿÚ@S¿Ýæ"Cqò¿ß[é€Óô¿æצ
4¿ïós_s-AGNbcu3FGL J1243.9-0217PMN J1243-0218?ïø$ÃÌÕi?N´PòA?Olð̪XA?N´PòH?ïü<8Õv?R¿Pé
9?>9W<Rÿ?R¿Pé
F?ï±N½?ƒVgä™T?ƒ¬zP¾¼Ì?ƒVgä™U?ïù^d2T?8Ò|
?J‡êo6®v?8Ò|;4FGL J1244.2-4956?練lû@)Ҟ²N©À:‰XÀ<+©­
å@Ê	rðb~@öäÎ?¸¯¤@î?›C‹p*Ö?âª''¥@ÉbŠ
à¿Ì†9•w÷¿ãª3z€Ïž¿çŸÑâ5iÄ¿ßk*ñER¿äóý">5Æ¿á…\€‰}BAGNbcu3FGL J1244.3-4955SUMSS J124422-495422?ïúV
ޝþ?@—)@ú¥?F§Ô…ˆ‰?@—)@úÍ?ïü™oÙ?^òÎÞͦ¢??Ó47Ž?^òÎÞͦ­?ïò ³!KÎ?cÁ|xŤ?Z¾™½hg?cÁ|xŞ?ïñ4‡‹^°?J!#,Ñ0?]–ðéB¢¢?J!#,Ñ!4FGL J1244.5+1616?ܛÄ-Š{I@SÂ=ÿ?àÀ:žÝõ<ôÀ<'è5Þß@l¦¿òÉ·@¨ _ñØ?»sLþ¶Så¿£1ÁKÂÕ?èIËÆ<Ó@€LÁz?í"ú¾z¿×9ƒ@;Ú¿áMÖ¸ª¿ãýR ^DY¿ÕïW¦°'¿åŒµ_ó°'AGNbll3FGL J1244.1+1615SDSS J124444.35+161621.7?ï´àqx;?wù•J[	l?'ýÇã¡ñ9?wù•J[	f?ï÷×Õ´èF?f
Ä~å|?PPT–/tž?f
Ä~å?ï³Ünˆb?e{9ÚW?ƒؤ]çQ?e{9ÚW?ï6¤æƒ
?†ˆ""¤©?™?c/žm?†ˆ""¤©4FGL J1245.1+5709?àx:¥ï.·@Mùˆ MÀ:>¢Œ‡b_À<¯è+Íä@‰€Ç»–@x\È_?»KË@ÁÍQ?¬ŠŸM/*?ñ××ârP@³£ùnìG?ïþÂ}¾qÀ¿Ø£k_I'™¿ãŽ.+ŒuÅ¿Ú~(Õ!°¿á©!âRðé¿ïÿâ¾÷!AGNbll3FGL J1244.8+57071RXS J124510.5+571020?ïÿ¤ é°?Ԙüƒë?+{âÉï?Ԙüƒ1?ïü;Êӄ¨?SPˆ&AkÒ?>!©cÚ¹u?SPˆ&AkÄ?ïí«w€?là2W¹a?büTñˆ‰?là2W¹T?ïÙ =¨|Z?^óG™?soá+Áѵ?^óG"4FGL J1245.8+0232¿Ù Ô¢ÚKÒ@PX4Á¨¬\À:ÒùXF3À<°·ŠEhÀ@‰Y"Eò¨@cIÙgåÂ?ÇҁÀá²?à©=EÛ¬d@U$¿ÒéG@-Äq3žé¿ïâ^¯c?ïEmþ
\z¿Ú!Ïþ°t§¿åÞ¯6'¿í8´FÄ	°¿ïýðƧÞAGNbllNVSS J124533+022825?Õÿòƒƒàq?ËʨA«à?å¾>È?ËʨA«à?çûä»W?ÔfÙ£H?Ð	Ð6‰Qà?ÔfÙ£H?˯lÄùS€?³5íS7üÆ?é$ÎÁ« ?³5íS7üÅ?Ù~Þm'?¶'ŠÍÃ?ã@Ézlu?¶'ŠÍÃ4FGL J1246.3+0112¿" &"&{@Pʽf'À;0íæ²QÀ<¦¦3
@ºþ‰³G–?ý*þE뜜?מքÜs3?ÎhìƒK?öz¬(©l@o…r›(¿æhŒEô¿æ¸Ã*Œœ¿ä÷'î\i¿Ä‹í¬vì¿åïw‡ R¿ïù}š_'7AGNbllPMN J1246+0113?ïþ¸ÇЗ?a¯m?(w?$sâöŸ?a¯m?(?ïýØØ?Uœe¬íg2?7ÇÑ?É=¸?Uœe¬íg1?ïà
´ŒLD?q#Çocss?oõKs³½l?q#Çocst?ïñlF"–?KD?Ð(?]'rØÓû¯?KD?Ð34FGL J1246.7-2548?ïþ¦bˆÍè@B‡jƒ+™À7]M•µ‹À;>Ð}[ur@õ@Lz@¶ŸÜ©¹¢?"i†<«¾?¾îܗ8@'w,¶Ap
@ð‰JìãC¿Ê,jÈÌ¿àf¤^ïy ¿ä؅½™©	¿åÿdd-§¿çȽ¼
¸¿ï(	3…iAGNfsrq3FGL J1246.7-2547PKS 1244-255?ïð/iU ?l'¤&j ?_¡ã-T¿È?l'¤&j?ï)(;´Õ¦?³BYTSa›?šÚø‰eKO?³BYTSa›?®wE?'Ä*æp?ŒXTb.¸b?'Ä*æp?ëOôÍÔ?µ°Ñ ¼?ÂÃè,ȯ˜?µ°Ñ ¼4FGL J1247.0+4421?ïРjlŒe@R0
ú/§À:j1ί%À<}ËÆ<Ó@ T¸?ú+Ì¢¢&?Ââg=Ñdz?ÂsLhckµ@óþº…¢l@šˆÙ-m¿í3e"¤7¿È[QIô•¿¿Ø¬@»1ý¿ÐÑÑCſܨݤ‹e#¿âüê×yÎùAGNbll3FGL J1247.0+4421RX J1246.9+4423?ïþ3A ?1üò/¦›¨?,΋ïÍçc?1üò/¦›Ø?ïûçòâ(?T3¤!úJ?@`4w_´k?T3¤!úN?ïêz.«÷?kŒÎ€MÑw?e…êÑTß?kŒÎ€MÑh?ïÓZëó‰æ?c9nèH?vRŠ;S?c9nèJ4FGL J1248.3+5820¿×'æ{æÃû@McáÁP—ÈÀ7²ÂFbÀ;QDy¬"H@#'0iK?üù!ÚE[T?"ZýU­º?§]®1S@lë5m @²ŒI¥¿ºOOŸx+¿Ü[é B*G¿Ý­2=>ú½¿ÙŸÕ]jo¿áGßÝË¢«¿à;‹ÇHÿAGNbll3FGL J1248.2+5820PG 1246+586?ïþ‹t±f?"ˆŒú̀¹?'OÈ´éšM?"ˆŒú́<?ïêÑbÛ ?öX¿7}?eù.$_I?öX¿7?ïä¯ÏÊÐ+?s½½Î¢ì…?kP05/Ôý?s½½Î¢ì? Öá?h
òa¨?~³¡¯"–?h
òa¤4FGL J1248.7+5127¿Á-BÕV—Ë@Pj:ÀÆ.MÀ:çÓƼ"À<Ö35·qò@ýV"U@sˆ€l¡ê?ÀOBßN…?  ÜÄf¢?Ðσ@;ÚL@ô%ä–.?ïúKUhè!¿æӀ y\¸¿Ømû:ôG»¿áTBý«'ê¿ä¬œ«¿Ð7h!&–BAGNbll3FGL J1248.0+5130RX J1248.4+5128?ïý!oR+i?0@Ÿk$)Ú?6ô…n¤Âª?0@Ÿk$)û?ïý˜"kZ•?Gón܆ D?3;d¥+N?Gón܆ 2?ïötªãõp?b	xÖ÷E?Sª8Ô?b	xÖ÷J?ïèµùIê¯?Píst‡?gJ¶Q5?PístŽ4FGL J1248.9+4840¿¬äbýpŒ@Qý`éNäÀ:½´ò»sßÀ<Ã9W9¢¹@=x±"ø@2™åﳂ?ÂxÛ^?«
®e?çˆäu_þm@)Ùçg'Æ¿åfH3ux¿ãn¯«SÖA¿æýh@[9â¿áV¨ž[¿ïΗÝ×·¿ï׌CoÁYAGNbcu87GB 124632.9+485605?ïý^{?3Ʉ‰55ä?5d'Ñ·?3Ʉ‰56?ïý÷'¯
?LòGþù?7ÐCj‡§a?LòGÿ?ïígk¯Üƒ?fëG
ž¦9?b˜"P#{ý?fëG
ž¦!?ïü‹¯?{µ?0ˆ6 ü½›?;¢†"S®?0ˆ6 ü½Ø4FGL J1249.2-2809?ç8˜VËHÍ@A\ÂzcÀ9óšw+À<J–6—l@4žm=ñ@/»õäô?¶ˆWQölÙ?¦
L46?ðÐÄ©Ü¡@!åÆüÌ¿âÚ%æC–X¿Ûhfç¿å&ýšÊò¿ÕŠJWu¿ã-ª}l'O¿áž¨âŒÒŒAGNbcu3FGL J1249.1-2808NVSS J124919-280833?ïù_óúǁ?CŽ ¿´?J€0áüÝ?CŽ ¿¶?ïýmÂÖï•?HYZŒIï?4'éHƒKø?HYZŒIÙ?ïóÈa3x?hèë%19ì?Xo=™Ñ
C?hèë%19å?ïÜOUË%?\–ßڎ'?qõØUmÝ?\–ßڎ"4FGL J1249.3-0545?íëçHw‹@L"V!uÀ9ìfknããÀ<)ñʳ@°5;Ì	?þ°ÆÜÈÃS?Àßäׅ?¿|F¢{Àk?üðÁo¡y@
óÍ]ìDa?±–!êá_׿҃Û!#f7¿ázá}]ù°¿ÝèèŒEô¿àáMø±W&¿èååvø…AGNbcu3FGL J1249.5-0546GALEXASC J124919.46-054539.7?ïúsÌFY¶?C{³nà_c?F0Îæ™$ ?C{³nà_q?ïü2ÛÝ͜?P)õãêy?>i!"&)?P)õãêi?ïå»bFê?sðמ-?jDù¹ä?sðמ$?ïîÆW†Š?M")Ç`?a9ÿ¨yvÜ?M")ÇR4FGL J1249.8+3707?ãñ—¤cÓ@Sÿ|E˼,À:5áŠëÀ<ZÝÌÏQ@ —øo'ßì?ú¤Ò—çè²?¾š½°û
"?»ÊkH£\ç?ùkøáþ9@v[»¹f?í÷G"êp¿ål­byFé¿Òv2â*'
¿ÆŸiýŸ¨|¿á¨[ý¿Ü'ÁM'AGNbll3FGL J1249.7+37052MASS J12494675+3707474?ïÿ9I^=?ŝoµ	?ÖÏÔ8=?ŝo´|?ïü«'Þº'?Oë'tð€?:¦Á
+uÊ?Oë'tð'?ïú«ÇL?H	ÒB%Í?EQøâϚU?H	ÒB%•?ïôûûóÐF?Aö¶Y%ë?V_r^?Aö¶Y%ë4FGL J1250.6+0217?åD,ÊVM)@PJ%®æ1ùÀ:7Faä ¦À<[DÐêh¿@Ÿ0'ü?ÿéki¦X?½e?½I?µô'žUk?øՐÀ­Ú@¦û˽Ù?Ú¿†ÞV&?ß¡B‡N¿äƒõ¶6ˆ¿Ù­K6_¿åÍF¿×ñĿُ­‡'›AGNbll3FGL J1250.5+0217PKS 1247+025?ïÊZ-H¤Á?w;ÞÅî?zÒé[­Ÿî?w;ÞÅî?ïÜù•7¿?ƒ†¦íá&?qƒ5d t½?ƒ†¦íá&?ïÎIŸ'?~BœñVüF?xÛ0wtí!?~BœñVüJ?íZˆç–º7?›"×bëbt?µ+¸ÃJ.A?›"×bëbu4FGL J1250.8+3117?Ü8¸k‰Ã@UuÎ1PÚäÀ:½^¿¨÷ÛÀ<³ùJ÷@½ënM'@dà?p?ň#û\Ø?ÀÇ`âÃÚ?ú4Q%Œƒ@—멱¿«?ïéæ]Â}é¿Êp¡Mm¿àÅîÁ껿çoñ)£g¿Ø§9ª€¿ïÿãzŽ;˜AGNbcuNVSS J125051+311706?ïúI|ÈRž?FeÚÈzæ?FÚÞµ"2?FeÚÈzÍ?ïû›•#"?XÓñ˜§b?C¥'«stë?XÓñ˜§O?ï¸_Ì­l?×æÀæÀ?èù¤ò?×æÀæÆ?ïÈJ×í?fÒéþŸ¬)?{Úÿ"	z›?fÒéþŸ¬'4FGL J1251.2+1039?ÖÚjŽo‰±@Raž­ÕÁÀ:È_Ñ÷®ùÀ<Ûž ç×@å•á"@CLŠÅÁ?ÊC#–21?³Øj9ڗ;?êÿ'>‰(@y	ڛ?ÌöÄŸä¿éØS³Ü:ÿ¿Õ—zEˆÓ¿ßѾmþ¿äóUÝ­Ô¿ãØr¥®AGNbll3FGL J1251.3+10411RXS J125117.4+103914?ïüó¶åBõ?PgcÖÇÇÞ?8bHÕèW?PgcÖÇÇæ?ïýDRyR?O­ÈZ6œ•?5Ýl7
dÔ?O­ÈZ6œ¤?ïø¥)最?cêû£¶¶?MkXeþ¢?cêû£¶Ÿ?ïñÄy5Ì?Dø³ãVÆ?\x÷
"g¹?Dø³ãVÅ4FGL J1251.3-0201?Ñ®¹ÀLS­@Nl)Ür\À9çÆaxÀÜÀ< ªÍÛÁ@Wš©+½?ÿ5}?Æ¿m?·íå᛻Þ?Ãð\žçaN@
–Õ"õÎ@Ú\`ˆ×?îÃRЇlp?ÀÁûxö¿àÖ8¡1=¿ãh&à>™™¿è	 B*Fû¿Ü.]Á&PwAGNbcu3FGL J1251.0-0203TXS 1248-017?ïåG†;Ì?gÔü
?j¸yáÄ4Y?gÔü
Œû?ï÷üüê?8?lQ:$?P+ñ?lQ:$?îĶdk\h?™Öüýa?£´™¹J9‰?™Öüýd?ïï}	í™?K:ÉÕXÀ?`'öêfî?K:ÉÕXÃ4FGL J1251.3-1719?К+¸=uÛ@FÆ~¿"ÀÀ:ƒ½‹ç)À<0'½,EÙ@Œ½T´¸.@Rå=Ì?Åi ÕãvÝ¿¯C²¡To?æÈa-A'?ý"ˆ'ðਿã)ò­1&¿çôáSlŽŸ¿èÖ¨]¬®t¿ïÿþó…õ?ïÿ¬ž5¿¿ïÿ±%§YvAGNfsrqPMN J1251-1717?ïýYºr?C«0Ó¥«?52,oC?C«0Ó¥«?ïãæèEºÂ?¤nŠ2f¯‡?lºE<â?¤nŠ2f¯‡?îïf¢šj?•ñ/°ïʕ?¡ù•ÖYd?•ñ/°ïʓ?ïöê˜Ìýê?T)­D?R*Îf,Z?T)­D4FGL J1253.2+5301¿ïRCwù$·@Pö¾7ޔÀ8¢}À;`F'µ@F‰!|?þæ™&­ó?äè!'ö?¶Ža¯Ž@}4ßݵ@¨ªƒ¡¶¿´wù
îE˜¿ÓFšDšd¿àíA·Zu¿àVƒ?4{¿ä\¼>4C)¿äCëGWLAGNbll3FGL J1253.2+5300S4 1250+53?ïïô\«‡?c+æ'=çy?`£Ty?c+æ'=ç?ïŸô¼Ý/¯?œõ'{'Ë@?ˆÐÈ´Ü?œõ'{'Ë=?ï é8¯?,՚@xQ?»âØêD?,՚@xR?íåÍÈ1? o¥.¢hë?·ÀїY¾v? o¥.¢hë4FGL J1253.5-3934¿Ëÿ8Ôæ)@7M‡ø‡eºÀ;Oô!¥l6À<­qGÏ¢@"RüÎÈ$œ?õ»
7 '¾?×(ª.'?ÞBãÈÂý@\ÝF—"@hU¥ÎÜ¿ääáÞ?¿ð?ð?Û襁6¿·d^ -¿æºÀZ΂¯AGNbll1RXS J125341.2-393200?ïùö¼>"½?D·®…•¥Y?H%­,?D·®…•¥]?ïú""ˆÀ?a}4'Uîß?EïõíÜú?a}4'Uîß?ï»H¿g©?QJðý?-Ð&9U±?QJðý?ïóv4ž@?Q­J›Ã?Y—ÖÃ]?Q­J›Ï4FGL J1253.8+0327¿îMuø},@P"3œ¾àÀ9vZT	lÀ<á¦x¥-@—˜épq'?þ¨S¦pA±?²\[J©q~?²ï'ó²ê£@ºÆ:"‰@ÂÂ¥V'1?ïæfÁ«¨¿Þlâ×P3¿ØÙL!–¨£¿âñµºa¿àajþütÛ¿ãIsÔ
3AGNbll3FGL J1253.7+0327MG1 J125348+0326?ïû> Ãmæ?@̪ä<Ž?C|òHm??@̪ä<|?ïñº]¥`?t`>9{ì5?]ЋDµ?&?t`>9{ì5?ïá
s&?yCI¸ëïÉ?nõŒb€ÙY?yCI¸ëïÂ?îëñ՝æ»?‰´ùؘ0?¡@â¦!"S?‰´ùؘ04FGL J1253.8+6242¿ïì­íüŠ(@K5ܜM©À:YÜë(À<Ÿ!ÿ.Hé@ì˕j5?ÿRþûB0?³Dç­†?—qd¤ÍÝÍ?ä
*àÔ@´@»ù¨M?ï§0ü!N.¿â®¡Óú¾x¿àý¢È6¿Øó"
3`¿ä¾‡Å[¿C¿Ú†«ë«µ%AGNbll3FGL J1254.1+62401RXS J125400.1+624303?ïþÕýOؖ?X–Î;:?" +v¬@?X–Î:ü?ïýWoÛÇÏ?MCí1í'?5D!Á…M?MCí1í'-?ï÷DJÂ??eõÎþÂ!4?Qwj{Ó~b?eõÎþÂ!<?ïüâ"f™?)Ã…m€g?8ëgÄË4"?)Ã…m€4FGL J1253.8+2929¿í¹k½W<@Uä‡Tów\À;¦JœÜDÀ<èdØǬÒ@ —aºH9?ô‡™Sù?à?…¡•ž?ÕÜ%³î¯?ó¬õ–ðqî@ Ü&$?ïúÁ.ˆÿ¿ïÌ{n5gÁ?è¨+b"Y–¿ÎfÆÞvB|¿áŸÂ¨†œ¿à×QÄòAGNbcuFIRST J125405.0+292708?ïûℱ7?Aœ§%•ž?@uí;#© ?Aœ§%•®?ïü€þ?V,6Îʽ?;ÿWx€ã?V,6Îʹ?ïÄA} ]3?‰éïä´m?}ßA/ÑfÑ?‰éïä´s?ïæ]ŒãÂê?[ìæ?i¢s=v?[ìæ4FGL J1254.2-2205¿â{¸²MÜ@DcÖ¶Zš€À:I}.ÿÇÌÀ<HéH-–;@g:<fã@	ýñ7?DZÓ!O°í?Èðužg´š?ÿ|卍ó@
Ÿ˜^†;?íŸ9Q´~¿Ý¯Òò䏿â0"刿àµ{!	¿åI¾ RÔ¿ïÒÁ££Þ—AGNbcu3FGL J1254.1-2203NVSS J125422-220413?ïâ˜å_K?mMŒû¶>Ê?mg ø³d?mMŒû¶>Å?ïü
£´±t?T
Â	v8Ÿ??ªâZt\?T
Â	v8œ?ï`Áêi?Eäi®§?"çÜâ¼ó?Eäi®¥?ï¾Ê¬D=4?dÛ󎪻?€MTîð²ê?dÛ󎪾4FGL J1254.5+2210¿ïOðº‰z@U@'(bõ™À9ÊôWÀ<UùK°Øz@¢v Ë@£iüóÜ?¶¢`<«¬í?¯«þöë"H?õUŒ·^¦@…Í»Š/C¿Î·_}>@¿æÕïUÑ¿Ùý"$½O¿Û…íÀ7h!¿çO;Ý%àd¿æp÷б^AGNbll3FGL J1254.5+2210TXS 1252+224?ïþ%Λ½?&‹{mf?.m£D:%?&‹{mf?ïû|䵌µ?VŸýC
sh?Bm)Í+¢?VŸýC
sa?ïñ4fÜ0?i±*hñ]?]—2GϞÍ?i±*hñK?ïçÊ^æ3ì?X'X)åè?h5¡Ì}?X'X)åç4FGL J1254.9-7141¿¦vÃT•ÈøÀ!¥{"ÛœsÀ9û<š»ÉÀ<³"&jÎ@l·2[ÇÒ@>öÞN«?¿j%®(ó?Ã?áD‡@làÓêÎ@®qLÉ\U?ïòr®sEr¿ÜC¬ýúl¿è$dIU´¿å{ඎœæ¿êˆè""©¿ß'ÿùtöAGNbcuPKS 1251-71?ïÛjìQ#?ŠLþˆœF?rwʉ×n'?ŠLþˆœD?ïü&ñ¼d?^z:¦a÷_?>Èrß6?^z:¦a÷^?îԉŸŒ#?–Ÿ7‰&×Ù?¢·f=ÏÈ?–Ÿ7‰&×Û?ïüy®Ë,o?+ˆ¼}ŝî?<2‰¦œ'?+ˆ¼}Ş!4FGL J1254.9-4426¿Ú3¿¨iÕ@2lYtæ[êÀ:DN®¹¼OÀ<;hë{ä}@vîªíÿÍ@Uçþz¿?¼ýòÆ¿‰B
ø'´‰?ʎ"õ"@ƒái\æ?ïèÝ¿cW¾¿á	Ê^ˆv‡¿æ`Ÿ¨žð¿åqž½c£¿Ö5ÿ€Ô%Ý¿ïÿúVrÓ\AGNbll3FGL J1254.9-4423PKS 1252-441?ïê½1!?bľ'³©.?eBÎíÞì"?bľ'³©+?ïüLvbË?V¬\ìrsœ??ýœLéŸÑ?V¬\ìrs—?ï¦ÇSïP?'°\–×k?†Î++û?'°\–×s?ïÛÔ)IàI?aRÒ3ýl?rë[Û¦?aRÒ3ýi4FGL J1254.9+1138¿ÅŠ,Vü±8@RŸ÷ÎÙ‡À9ýpƒöš&À<;á~4¹E@…6»©@õ–AöD•?¿Rj,d¸?ÊÐfŠM¡?ÿÀÑìÇ>@
©ØÎã¨[?ÙO³œz¿ã³ü†Î»º¿ëò…žeh¿è¹F¨Zý}¿à×Ë~3Ó¿ïÿœ,ñВAGNfsrqON 187?ïÉãPRâ/?~}ª¦Ñ:?{W֎çþ?~}ª¦Ñ:?ïô«Ãć?t¨kmáñ?V©Üxvó3?t¨kmáí?íÅj•Ü
6?£aãÀíz?±Ô«Q–W?£aãÀí{?ï†g4ýa?€¬6í÷pN?Žæ2À¨?€¬6í÷pM4FGL J1256.1-5919¿×
Àƒ(t@_0ÓÊÀ9Ç\ŸTÀ;Ï©mL3µ@ uxj…@újÊy5v?¸Í¡Þây¿™4YªÓ?â#Aî·Ù @B2<h;(¿ï¼IýzÂ?î—È©Q'¿æµLG×/&¿ÞyÀGƒL¿Ý€&Ö@¿ÞêiÀ¸íGAGNbcu3FGL J1256.1-5919PMN J1256-5919?ïÆ7ßø?€³Ä—¤?|üudû?€³Ä—¤?ïãKiµ'?—çwÿÕò?l´–bJo?—çwÿÕñ?wË°>?ˆ˜ Ÿ0¨|?ŒSâ
ð"?ˆ˜ Ÿ0¨?ï«Êþ+Ð?wðŽ£^9Ë?…
@u<?wðŽ£^9Ì4FGL J1256.1-0547¿íðóóã°E@Lˆ'ùD$À5…¼ÇœdÀ:}2ñÄÓÚ@"¿/üÈ@'d¼B;?y@X¿	?²Û''ãB@0­ÇGQÎ)@$ ?ö¶¿ËDYv=ôØ¿áVƶ2W¿å='AŽ@¿äsçŽ2׿é=Η¨(¿è·_èã«AGNFSRQ3FGL J1256.1-05473C 279?ï ùæž?…ïºZþ¥?‡à†z˜Ÿ?…ïºZþ¦?à f?£}S8?Z÷ûæG?£}S7?îúråi¤?š+ÌÏ©? Xѯ‰eº?š+ÌϪ?¼%¤?«n¥c%?¥tOô=¥Å?«n¥c%4FGL J1256.2-1146¿ïêOq•–@IŠ<æÁÀ9r‹ò)ôÀ<øð@€-.â@§?þD
Öó—<?¯@ÄkTa×?›×Ù½˜sÌ?ì'Õ ™@cO•Gû¿ãèÔÀ6;{¿áKû¡K"©¿Ø}ŠDg
*¿à‹ã˜Á,†¿Ú…뜛¬™¿á¥sŒ¿–ƒAGNbll3FGL J1256.3-1146PMN J1256-1146?ïï-^ڄ7?Vä›+PFF?`Ò¡%{Èk?Vä›+PFD?ïøŵ(S:?`×tðWô¢?Lé+^³O?`×tðWô¦?ï­cLHn?"¸¶mµ
í?"½ç,íäR?"¸¶mµ
ï?ï•ä`—§?yéÄ?•5z?Š†çàK?yéÄ?•5w4FGL J1257.2+3646¿ïRX¦8Ö¡@TçÿX:TÀ9à?d‡À<gñBÍÚê@1ÆöI?þ¨™Fƒ?·›"™ÐK2?¹v´è)ŸŒ@Ìø×Òª@
ö8#¿çtØïð¾D¿×šƒT]Ð¿à¾V<"¿Ú«
š¸¨~¿æ~VG4qø¿ápq·Ó@"AGNbll3FGL J1256.9+3649RX J1257.3+3647?ïþ‹Ó†íŽ?!oüÉS]?'BǑ'!Æ?!oüÉSP?ïû•NÍv—?Tš}?Pæ?AªÄÊ%¤}?Tš}?PÓ?ïí'ð¨Æí?g
-F¹…?bmW9'?g
-F¹"?ïé§'Æ¤?T"%YIb?fXØr9[t?T"%YIQ4FGL J1257.6+2413¿æTiõ±ÚX@U±Eà´áÀ;̀üê¡ÊÀ<Ûû()êµ@"1Žw&¨
?ùb¡ Ï?Ó¶…">C]?²Ýí§^Ô?àyt*tGÐ?û¢Ü)T?Î<©Ôz@8¿í¤u•®RŽ?ªá¡½våÝ¿Ú
÷À@wi¿zQ–åNË¿á\ǶãV|AGNbll1ES 1255+244?ïþ½Tž
"?÷jî†èÓ?$*¶-Ô¡?÷jî†èÝ?ïû¼Þ	ô?a?rYtR?A‡Ø/'
?a?rYtL?ïôܧzŸP?UѸ"#?VF±
ÁbB?UѸ")?ïãNg80!?a'¦Ü+0¡?l±˜ÇÏÞb?a'¦Ü+0¡4FGL J1257.8+3228¿Ð'æ"ø\2@UwîN&ÕÀ98dUêî À<	*	¾Å£@|%ÉX@À«;'?«Û¡&ŀ?ºS*tr×@µ›Á'@'ãçp'?ïÿîbHÊt¿áû–ä³s_¿äDÄU/¿äÚ
\ßÔç¿ê9yh¡ª	¿éN‰€Fâ=AGNfsrq3FGL J1258.1+3233ON 393?ïüŒ@
š°?8ÿ‡ÿi/–?;ÿ"*wg?8ÿ‡ÿi/v?ïø^‡|ã-?clÔ=YÇ;?N…âsL¿?clÔ=YÇ>?ï9€™ñ?'˜G.ú5^?˜ÏìÎގ?'˜G.ú5_?ïüÌQ짗?+!c9ãW?9pšÃ??+!c9ãV4FGL J1258.3+6121¿ß.㓁‹¡@K߆
¢À;K›	bÀ<ò"Ì@"öàqšL?ýwœiW²n?ÇÉey¬iU?ÅÚyMBÔ?û$Éþ¼3"@§éÙM
Ð?í
z<@Œ?ìŽù,§'ø¿Èêû÷\ÃO¿Þêz\½p8¿äQÁÞÝ£¿åé÷ 54AGNbll3FGL J1258.0+6120NVSS J125820+612049?ï'ÔM½(«?‹Ì.0 :õ?‹J쐵Õ?‹Ì.0 :ø?ïébw?}¿ßkŒ?fbü?}¿ßkŒ	?ï©CöiQ?'r䤆9€?…¯<Be«š?'r䤆9?íՅí%a?šÇˆ[§?±SЗ¦Ôó?šÇˆ[§4FGL J1258.6-1759¿ê4Éî@FkÇÞP'ÏÀ97-Xþž×À;êU'þ@'°«@ݝ«w?°n²ÿàå!?Á–€JGÖ@I¬¤j®@[Ñsz¡?ã·íu?¿Ý`¥\E{4¿åµÔ}›6R¿äýÄy¿êéý)‹ê"¿ïÿùStAGNfsrq3FGL J1258.6-1800PKS B1256-177?ïØQJ?Z…A?`ld'®µ4?Z…A?ïùKƒ¦?`E
H¤É?JÑñeÃü?`E
H¤É?ï=ôËgø?˜tTšåÔ?˜Af"îR?˜tTšåÔ?ïø;戻q?<Ð-žIñ?OeÝ=o?<Ð-žIØ4FGL J1258.7-0452?¬‰›ö"Âý@LúRv‰ÊÀ:Úž´æÀ<_ãåî@!wãۇ$Í?ú—FBÐ?ÊRøur?Ìçø··;ì@Îå«Àä@‰þЪþ¿ãtyŸ(NÔ¿ïÿÉy[5±?ïÿç¬L#Å¿Öèq²Ë¿ÜŽòâ
K³¿Ý»u›AGNbllRBS 1194?ïý@(x?7Kvèõ"?7åÿ6¼LH?7Kvèõ¯?ïü%ˆ[2‰?QíX7 ?>Ó½&k»g?QíX7?ï×ÍZº{8?weÈRÁOk?tR¢ÂdÛ?weÈRÁOm?ïÚ¢#£V?cÑh
¾¬?r®ît.T†?cÑh
¾¦4FGL J1258.7+5143?åÄrí2Š´@PWÀÁü2À; ¼£‰ÝdÀ<¥~`X/l@1ˆ°h=+@懖ü?¼žWµs•¿·QԞ}Y?üÚÕٻș@ÚÉWLm?í}î¸u'¿ë¬dAÈø,¿è†çn2
¿Üë›D«¿ë/˜Ÿá²?ݘœä§´åAGNbcu3FGL J1258.7+5137NVSS J125825+514225?ïÁ³»¡'¨?|Ž#=8É?&"/>¬?|Ž#=8É?ïÜ¥þ¤¯?—hçe/Èb?q­­ô¨¦?—hçe/Èa?ïŸ/S­?†ÛŒÂ'F?ˆ4+8ÔÑ?†ÛŒÂ'J?ïˆé¶ŒÐ?~‹ê«±ôr?Å»\ÌV?~‹ê«±ôm4FGL J1258.8-2219¿ì³¬åKÍ@DA¸d"À8ŒR7Û9À;‡Üßi‡ƒ@ÏZ/Kr@¦áÞ¬É!?¤h_ž¡?·î…?€¯¤@¶æS†Ò@ínοÁ!¿Ìl•?ì+¿â8ϟý¹¿åg­Ó
¿æZ§K39¿èꀥ+ô¿ëʶDËAGNfsrq3FGL J1258.7-2219PKS 1256-220?ïøn¹¯?BӔú´/õ?OöE¥F?BӔú´/õ?ïö¼;ß[?mt¯"båŽ?R‡çˆAHÃ?mt¯"bå?ï½úQÚs?€l'ȾÔ[?€k¹Icƒ?€l'ȾÔZ?ïý~xJ´?'^óFŽæ?4=ª_ü÷?'^óFŽù4FGL J1259.1-2311¿ì<-(ãÜj@Cґ!%¶À9'u°ÐîÀ<
ìíԄQ@Ab…Ü#@Tò»sÞõ?¶‹4|?¥0â嬱?ëÝ[IŽ¿@O×X›Í¿ã‰è‹o4¿Ù£¤ÛA¿ã]'âïj¿ÚZ›WûQ¿å<á1ޟ¿Ø'·þ¯AGNbll3FGL J1259.0-2310PKS B1256-229?ïþN#ß?"ùik
p	?+δ(?"ùik
p?ïýh´ÏÁ?QVŸ°š^Ú?7DºYí›?QVŸ°š^Þ?ïõ3–ä?d]³Â܃8?U™ÚÒ7Ã?d]³Â܃5?ïþ^Ü-?¹çä8?*?ý(Ñ?¹çä'4FGL J1259.5+2332¿êGª—IV@U~ªâ—9mÀ:ÎdÒ°,À<D(v@Îý@¯Ígý?@ÍDƒ½?ÄBðëe¿³t¬¾ÿœ?íä¦Þ%»?ÿ.¾+Ê3?¿â‰€Ç»–¿æØ^NêÊ¿èïæb.ï¿æûƒ¶¿éO}¶åû¿ïÿò~#¿AGNbcuNVSS J125936+233047?ïñÕKÍÑ?^èqU9ÿ¥?\Uhd]ÃÁ?^èqU9ÿ¤?ïv¦¬?<É?¥È5ØU´?'+*xfè?¥È5ØU³?ïRj¿£È(?‹t'ûa?•²¨†úÅ?‹t'ûaˆ?îœsÐC/¾?›,LyÿF?¦8ÂûÍ:?›,LyÿF4FGL J1259.7-3223¿ïû;]|X@>r螺jÊÀ9{f¶~¢À;ðítA@èU³:Õi@–ªú-´?²=å~I‡?Àf0 .H¾@
Ä.béÚ$@µ¬]@¢Ý?ïû)ƒ£8¿Û—\¨wƒ¿æW!U;œ¿ä]sYN¿ét7	‰¿ïùûn Ç‹AGNbll3FGL J1259.5-3231LEDA 4075145?ïï'߆Y?`»aK0)?`} yã§!?`»aK0'?ïú¶}Tˆ`?eþTÑ?E&
­Þ'Ë?eþTË?ïf¹íì?'ýâ¶R)?ó(ÂBn
?'ýâ¶R*?ïôvî2ð?Dƒá%ý?W#šÉà?Dƒá%ã4FGL J1259.8-3749¿ïûµáâtC@9²c"úÎÀ9©N¬5}À<4\¬©@×@û6½\@΀ÌC:?²­¢ bl?sLù7üW?¿3ƒåþ!.@2Xª'
¯?ïé»ðÜvŽ¿àËXߕ&¿àߪõâoÌ¿á‹}w$$¿â፞¹"¿à®þúGAGNbll3FGL J1259.8-3749NVSS J125949-374856?ïû•&š‡?9fA)UØ«?A«e—õçP?9fA)U؍?ïýÄ=ŒÓ?J4#è3D?1Þ™g¾?J4#è3T?ïí³Àͤ"?q2b-]¿?bL?2[m«?q2b-]¿?ïíX^©yü?P°&™n§Z?b§¡V†ê?P°&™n§O4FGL J1300.0+1753?ȗaS¶ò@T#ôörÀ:¶K̇,°À<|÷¤ëá@
º´2w@pÂàºÀ?ÃÆæþ¸?Ÿlp&궩?Ônw⏬±@›îÀèh	¿ì'+ˆDÀ?¢›+Ñ¿çØs>f6¿çE)Õ¼_—¿ïÊù=n˜?íýgŸKŠBAGNbllSDSS J130008.52+175538.0?ï¡:ê"Ë?Š,(•qu/?‡±|E[
T?Š,(•qu.?ïöI(‹+?g{œ2å?Sm®éͨ¬?g{œ2Û?îÑ
µìÞ[?"'¡?"V?¢ïT¡2J?"'¡?"T?ï·¶ò	'?v3²»j?'C}›£?v3²»m4FGL J1300.4+1416?ºLy"`@S>iƒQYÀ9tùòŸÅ-À<<Šk(m@_öèª"ÿ@†dÆS6?±—"–}/?µÝ';¦t?ûÌO~ÃT~@j«²¿ËÜNõÜeœ¿æ£¬!Üs´¿êHõ!¬‰¿åòI(gþ¿èò%ìù'þ¿ïü±®¤AGNfsrq3FGL J1300.2+1416OW 197?ïùOçW
?GøÝ°­?JÀa¾£Ö?GøÝ°«?ïøÐéÃ'?fÔ¯à)¹'?L¿äXó^?fÔ¯à)¹Œ?ïªÆRvÛ?øõw¼¶_?…ŽkbHï?øõw¼¶Z?ïµÚSE?s¥Šê{f?'‰yë8®¼?s¥Šê{f4FGL J1301.5+4413¿ëx;D´ÎÎ@R1×Ûô‡ýÀ;Q3Ï:eÀ<×ÊZ+Ł@4ºuÝ&â@i[»èxû?™ڇ™x¿ˆ»Ö
ù3?ǵ­áÐ*@/xº{çW¿ë‹hH¾µ³?濞`¨·D¿ç£õ¾¸¿×|ÅW7Ÿ¿èŸÐ_©]Ý¿Å[¿XðÜ÷AGNbllGB6 J1301+4416?ïùZ´4 ?MaÀ =?J•/ß-z"?MaÀ @?ïýðO«?S¦–iÛ«,?7}‡Ú«"?S¦–iÛ«5?ïÇE]ŸVÃ?~¼ÔØîó?|]Q0Tží?~¼ÔØîó?ïø©%e¼??î¹àÖäà?M[k†i??î¹àÖå4FGL J1301.6+4056¿Òq¤Ã¾@Siì,äeÀ;*@tdVÀ<Ö=Jä*@ &H½´"?ý
‡¶B?Èr_™ãA?½N䔔¢?õ")'°I	@µáL‹žÚ?¸f§>r×c?îŽCû"¿ÈydDùb¿áR"!7]9¿æ½+o"O?±Ô¼ZcαAGNbllRX J1301.7+4056?ïýb¨hh™?5©•ù7Y0?4ê¼¼»5:?5©•ù7Y$?ïü2'—?Uïg$OÙ?>o›sN¦?Uïg$OÑ?ïæ…Ì"F§?rÚԚè7Ä?iz3k¹Y'?rÚԚè7Ì?ïÅyOÆs·?jµ&në ?}CXÆ%?jµ&nëš4FGL J1301.6+3336¿ÝœÏ¢¤@TÉØ­«ŸVÀ:z/w¼ÐÀ<t[íf H@êÑ;F}@cH9Tµd?ÏAQ'Ó?®…-âønw?æ}+Ç.'@ä-̖ñô¿çºÂ^3çä¿ã1¹€¿®¿æšýqÛ:¿èO–áXu¿ïûãp}@¿ï´ÉÀþ¸WAGNfsrq3FGL J1301.5+3333MG2 J130126+3337?ïýåÕ·™
?- ˜Hòõ?0ÑRC7ª?- ˜Hó?ïüdzA‡È?SdÍÍU6?9ÂeóÁ¿Ð?SdÍÍU;?ïéTÏ3Å?hOŽ7(æR?f«0Ìå9G?hOŽ7(æ`?ïèÂ-þ·Æ?X…kö¾>?g=ÒH9¬?X…kö¾D4FGL J1302.3+6901¿ßÌG/(@H:}ªOÊÀ:ëè&Åf§À<ʞc,ö@bdþ²M@›?{@?ÅM%ã‹"?¡ðþ…V—?ÔhöÎþÖ4@UÞÂî| ?î²k!·	í¿çM³9ä'¿è-ê¿îI
{^¿ÊϵŠeõ¿ïþ2Àœ'ÈAGNbcuTXS 1300+693?ïþ¿†>kþ?+Ñ@¸X?$œ@'?+Ñ@¸C?ïû—‰"‡?cÑíÊ@ù?Cý¡Ùíã1?cÑíÊ@ù?ïÇ=ê½?}ÞÁÁtß?|aq
ò¡™?}ÞÁÁtÚ?ïïs>pl?W:ÑُI¶?`ŒÁà?W:ÑُI¿4FGL J1302.7+4750¿Ë™]‹"™4@QJS5À:ûâTôNÀ<¿cí@»õÊd@Xb—¤Í?Ä|`8Nû翶µ_©D?ðùV̕o@'âý:Ó»?¨gmޑª¿ìˊw½¦¿¿ç§{9\B ¿áÁCâWùf¿Û!²Ø/Ÿ¿ïÿÅbu@AGNbllTXS 1300+481?ïôÞmsw¬?[ùÀ'S?VC%§Š?[ùÀ'S?ïÜgò`kq?'†Öm؉û?qÌÏÊG??'†Öm؉û?/óJÍ?†t'‡é'?t-LÅ?†t'‡é'?ï§úö²Ïh?€
¡ÄBŽý?†BSL%Æ?€
¡ÄB4FGL J1302.8+5748?ê!В@MŸ©\…<À:W8õêÓHÀ<¾r¡L%@ÐÎý'@Y?¼®q˜?´B®Ñ9C¿5¶p?I?åÃ"ÿßHÐ@sã*\J?bmˆo¿è=þ"Ci¿àöÝâžÆ)¿âEbk¯ü¿âe!«ÌL¿ïÿÒþÀùAGNbll3FGL J1302.6+5748TXS 1300+580?ïü™\OøL?8.båÜ?;5€=¤¥?8.båÖ?ïýŽE`ýÞ?FÂ0†¾6%?3ÔøÞ?FÂ0†¾6?ïß]CX™l?wÉ\_#zó?pQ^S³J?wÉ\_#z÷?ïø…M(ý.?:dSåZ¦?MêË\G@?:dSåZ€4FGL J1303.0+2434¿ëy¶-f˜@U–Å—Ne¿À8Ì£Ho›À;ÃÀ…–­V@u¸"Ú¾@‡5ÜZßJ?¨ÎƒKŠ©?´Ýv=I¸@¦˜5‹'@ÎØÈ-¬?Óe±ÀVò«¿Ú¡Q¿tè¿â™ÀGƒL¿âUŽU™¿æ@&Ì£¥¿ëÐøÀñwQAGNbll3FGL J1303.0+2435MG2 J130304+2434?ïû'²Uؕ?9!R²—?Aµ6¨©=?9!R²z?ïù®¾>j?\/*Õá?IG¡WÓ?\/*Õá	?ï¹3«Ú(?ƒí{…êõ;?³?	v ?ƒí{…êõ7?ïúRÛ9+	?7	«‰=·?F´"SØ?7	«‰=·¨4FGL J1303.6-4622¿ít££Fà@0s§ü2ëæÀ:±®£íÀ<AÓë¤ÿ(@¹èÁÊæ@¿@D"­Ç?¿—ç'ËÊ?Æ"ïĦ¯@ˆì9ò@fš%Ç:?ïôÁPlÕ?Ïv<È2^L¿ß—dqē¿åˆabñfà¿è×a {{¿äoØ ?¦AGNfsrq3FGL J1303.7-4619PMN J1303-4621?ï~)ë
?‹â+Ӏ ¼?:œ]~¾?‹â+Ӏ ¼?ïô
~
I·?€Mͨ=Ž?Wëël'œ?€Mͨ=Ž?í·©ä‰Ìƒ?¢
çê±ß?²B°Û±›æ?¢
çê±ß?ï֎ӲЅ?a0w¼Ò?t¸–&—½v?a0w¼Ò4FGL J1304.0-5539¿ïÿ%¾-uÉ@´Ì?ß À9ésÉ%x`À;‹)ƒ‡@äŒu™µ@1;â.^?¼a™¢þÈ¿§ïС²[¡?ç2t[òo@›yòŠKž¿¼Ÿa.Ä
¶¿ãk›ŸXJo¿ëÐOt…
¿ÝC =͕õ¿ïþ"þ?ïâ
;Qå¦AGNbcu3FGL J1304.3-5535PMN J1303-5540?ï×í¾Dè?€Š¬«q0?t	 Ýñ@?€Š¬«q1?ï˦$?Ÿô²!ê8p?z,íòyðÅ?Ÿô²!ê8q?îpÍÛ?š¯žŸ9£ž?§èó/Ž¢J?š¯žŸ9£?ïÙՇd,i?f+GÚ?s<MéË-?f+GÝ4FGL J1304.0+3704¿ÖÉMØ°@SíKƧïžÀ:ÚñfàêÀ<žÈ:£j@Á›÷—ј@;^ʐ²?ÆcÄÄ?±h^ÊKú?æ¢6Æeª@¹©ñb?ïûùá
÷¿à™Ò¤}"¿çڄßÄK¿á¦W¸M¹Ç¿ëKz‡…šß¿ïØODù"AGNbllWISE J130407.31+370908.1?ïù'£·¥½?L"99|·ú?Iµq!i°?L"99|·Þ?ïý5½ò?P{-ÐY}?6Wàl'?P{-ÐYp?ïDZ]Iüj?€±&x ÜÒ?|'Q[Êý?€±&x ÜÕ?ïØ:Ӈ~¦?b£æ/jëe?sâ–<@¬æ?b£æ/jë`4FGL J1304.2-2412?ÖÀ¼Ib•@CH×ðí=†À9Ëúú݁PÀ<(ÒO̲@÷õÄè5?þNŕ æ•?¸òƱ¿S?°­Ù'è‹?÷OÙý6÷ä?ÿA‰BŽ?ë\|m8è¿Û¸¬Cë<O¿âkb^ÄÜh¿Ø6%€íü¿àk'³ò
t¿á¶}euüAGNbll3FGL J1304.2-2411PMN J1304-2412?ïèÂÿ*¦>?[8'óÿÅ?g=ÕYÃb?[8'óÿ¾?ïÓl¦Æ?‡ÎæȔG—?vI¬ü1—?‡ÎæȔG—?ïÏR¦ÈÉÉ?wCPGÃGû?xV¬›› ?wCPGÃGò?í_Ý]óñ/?•P¦Bˆ?µ`vŽ?•P¦Bˆ4FGL J1304.3-4353¿éY¾/³[@2êœo6ðÀ8zËïW;PÀ;wg)ÚÄÝ@E3'¹XQ?ûÎU}àÖo?¥Ø‰n~7é?¸Lݾ·‹G@ÅO±@|÷xÇçá?ïéXÎG ¿àùoߌ¿Õf¸Ü*ï¿Ú
ƒ÷ÿ¿àƒákÀB{¿Ý_ò.+AGNbll3FGL J1304.3-43531RXS J130421.2-435308?ïþéÕ"?o"6?!b®Ö¶ýÖ?o"6
?ï吒{n¸?dþ­H…?jom"'Fí?dþ­H"?ïº
¶ïh8?…#q?TK?}RD%ò4?…#q?TF?ïá$ÇãŸ.?V'(™å?nÛ8`Òf?V'(™ç4FGL J1304.6-0348?»žj»©@MrK èBtÀ;g€t.¦À<¥Ó`dĦ@?d3?ýùÓ`dĦ?×@.C_PH?ß× ìt2?ýŽ0"óA¬@	/^Ä;¿é«æ¾š¨¿ìì©@։å?ýz¿ŽËµ¿æI;þ]éj¿äþø™q¥¿ïÿYFÃ2ðAGNfsrq3FGL J1304.8-0338PKS 1302-035?ïüþ5nÑ?7õFDé?8W¤‰?7õFD®?ïý=u	(?MçðZ¦q?6W·>ÁÔ?MçðZ¦"?ïXGÞ)U?•k"

Ô?t÷:ÕT?•k"

Ö?ïä¡`w?W¯?…Ò#?k^Ÿéˆîî?W¯?…Ò.4FGL J1304.9-2107?ç™çÔË_"@Dл¡+^SÀ:bßÔçM'À<>-o|@š,œì	~@2ç-¡"û?Ä_DB™®?µÏžcWé ?ï'ø!dS½?õ¿Ý5¥©?î.Iq?栚tŠìX¿æ:)Çy§¿ã"9°ûµî¿à‡Ý~›<¿ïûï< AGNbcu3FGL J1304.9-2109PKS B1302-208?E:»?ˆçê/G?‰Wn±Q8w?ˆçê/G?ì»úþ¹ú¸?ÁÍáÞ×J?º (
0*2?ÁÍáÞ×J?ïloµÞ´ì?‹"'ú9Ká?'r	D)b?‹"'ú9KÞ?åeí\oæ?¸•E€£QH?Õ4%G!ô1?¸•E€£QH4FGL J1305.3+5118¿Â5•i¢žŽ@PkM:'£À:îòüÀ<Å'o(­@1æ×æ@;Ù_'F—?Òü4g??Ý_+ÿ¸1Š?úY
wt¬@ò!°~ã`¿ïûUá³äž?ïcóÅ_¿ìoC"º"¿ê§Š$Ô¿á¤jB"ùG¿ïÿ³ÿÌS€AGNnlsy1IERS B1303+515?ïï8ÓÙòž?lf^™Šæ?`Ç,&
c¼?lf^™Šæ'?ï̧-?•a8²Jha?yô¬8}é?•a8²Jha?íL*ŽÊ8?£iQŠ/Ú?µž«‰«J?£iQŠ/Ù?î•VèI÷?šG9˜bä$?¦ªž±{`€?šG9˜bä#4FGL J1305.6+7853¿ì©Q§"À$@CÿyÈCÀ:EFmCÐÀ<¯:ঞ@Œè0Uˆ@ðàpÀ?¸­G`ç¡d¿I]ÏÖüØW?¢Èè!ù
T@­˜¤§Ö?ï]=Þ1ùø¿â²ªפ—¿ä'›…,$K¿à;ú'½˜¿ç»üšð±®¿ãÑqw; ÀAGNbll3FGL J1305.5+7854S5 1304+79?ï½4R
*?|"
^Ä3Š?€²ë|ºu\?|"
^Ä3Œ?ï÷©7+jð?kñÚrBGC?P­'©*@?kñÚrBG>?ïºJ"Ū?'§Ùí%Ê?mwN•_Ö?'§Ùí%È?ïzúF–£"?z§Â€;½¾? ·-+w?z§Â€;½¾4FGL J1305.9+3858¿í=s,†"¦@Sq€ˆP›úÀ;"Á¯bX»À<ópˆÿ£@™¶¯T@·
è`Ý?ÍSÄ[d*?³G`ÖsY?å)¦¢@²"@ÖAj®u?ïúÀ~gå¿è™K`P¢°¿Ò¦…eZ!ß¿è17æ Zé¿ì;yÞhUª?âɛ?-±AGNbll2MASS J13053124+3855218?ïûN[YJ'?D>K"¶'?Bƒš×bÄ?D>K"¶(?ïü.YûX?U Šîñ0?>7%A®?U Šîñ0*?ï`ô?ÿ?oË3ÇÅË?"áx /?oË3ÇÅÊ?ïÓ«:%mõ?fþÓ墥?v*bíIp?fþÓ增4FGL J1306.3+1113¿Øc­xÁRé@RmÛ"Ðå`À;1Óºý—À<£Êz5˜@ }¹!]¹?ÿÀëíúCþ?ÅџÅW¸y¿l‹.|'3o?¤ëÜ1™«@Jc]¿ïÿý±q&´?ïÿáÍì¿Ý ÎâP¿àÅ%ƺd¿ïïícEI¶?ïYà37AGNrdgTXS 1303+114?ïõþJ®¨?Uo$h;?Tkð¢¯
?Uo$hF?ïú`ví?aµHê\{ç?F–'¼N2?aµHê\{ê?ï™-œ«?•ñÊWÏ.?žßLj±?•ñÊWÏ0?ïÁ0v;à?v֊þÂ<?gÄôâÙ?v֊þÂ<
4FGL J1306.7-2148?ï1¤"Wtà@DuöM½ùÀ9ó~°à<À<,YÜë(@s{ϯ*P?ÿ³!Dô%×?ÂGFe•5?ÉL²`9ü{@¶n¡žJÙ@ ZÑ1áO?ïþá77¥¿çšf³"?ã¿Ðƒp!ûþ>¿á†UºF¸K¿éi¿·:"Q¿á^˂Iñ¼AGNrdg3FGL J1306.8-2146PKS 1304-215?슃*Wó?¹ ZÀ<w?»«æ¯}@p?¹ ZÀ<w?ï_¼«1ïd?¢Õì™?"j™Ây?¢Õì™?éæ{˲
?²‹}ç†G?ÈgžÑ7Ë?²‹}ç†G?ë£h|5ÛE?¤¹" @ë?Ár^('í?¤¹" @ì4FGL J1307.6-4259¿Ìºð÷«Ì¬@3ÇÅ£ãŸÀ8¦17°pvÀ;¼-Qqâ›@Y24…˜±?þvbBw†?¤­r¿e00?žN%ûÎ?ö˜l¨ŸÆÚ@	É~8À¿ØàᬭȿÍc)Å÷¿Þ$_۲ĿܯD3‹ž¿àÛçQ³Pû¿ÔcÛÝrAGNbll3FGL J1307.6-43001RXS J130737.8-425940?ïúS$QØ?B(vR‰?Gò³n¸¢K?B(vRˆí?ïõž:e·ø?maÒMm?TË4‡?maÒMm?ïÚ?ý÷L?}dpN!dÑ?rà8Yã?}dpN!dÕ?ï¾Âc#?oÇ`Y–å?€Où'7"?oÇ`Y–è4FGL J1308.4-6706¿ï©LÎô€À*"'AÀ9!'ˆŸÀ;™)†âñ@ J5Ù*Ô@½¾hê?´uÞÝp‰?¹YÝìÚ´A@ÿ}>@C@ké?Ÿ'?îçuû.ßç¿ÓЕ"60¿ä¬j¹¦¿æ:"`R%<¿äXÞ=¿ïÿÿ" 5•AGNbcu3FGL J1308.1-6707PKS 1304-668?ïý¿¼ë?+àtmœQ?2* ¦‹?+àtmœ'?ïü}÷é?^Ž3ôFÙ4??ÇL@¸F?^Ž3ôFÙ&?ïM|p}?^8¶°?–P°ð@?^8¶¯?ï÷0æeðM?BÊ«Æ*?Qž34f_?BÊ«Æ*	4FGL J1308.5+3547?è©+(WØ@T&»ó¡MÀ9ëÂÐʈOÀ<f½Ž©|@j°†5á@tÌ?ß ?µóÁI5ÿ?Í[‰ûkò@¯ÿCAž@Z3k	?ïnÙgÒ¿ÚÊZ+ŀ¨¿ã¼œ2Ñ
¤¿çGÏ[¦¿ëä¡ÿ¿ïÑ ;tJAGNfsrq3FGL J1308.7+35455C 12.291?î#cÔژ?©!˜¹·-?­É²V~»?©!˜¹·-?ïðI(4Ó?qvH}Ò?_m¯Ë–[?qvH}Ò?泊‰;¡?³"¾òfü?ҘëÚ툽?³"¾òfü?ï¡GŒÂ€?r²š@oþ?‡®Ïßæ?r²š@o4FGL J1309.4+4305¿Ôù!†q'F@RhVWûi˜À8êé—îâÀ;ʟGX"&@ðÀΑÈë?üMJ†6‡?§xæàcr?µb»¶úÓp@_$•á~5@aÁŸÈê?ïêv–_Rv¿ØHŒ¡8ŸY¿×4B<e‹ö¿Û}»ÂŽZv¿âÖùvy!¿âçrj€§ZAGNbll3FGL J1309.3+4304B3 1307+433?ï÷ìÞ¼û?RU:>¶?P&Cà†á?RU:>²?ï¾VLܵ?¦v(;‹r?€j_¬ÈÒÛ?¦v(;‹r?÷ÉâÛ?ŒväC;?‹
‡I)?ŒväC;?î±¢å?'û³·¬ü8?®dåÞÞQ´?'û³·¬ü84FGL J1309.6+3718¿îwÅ~²ñ@SÇiÂ;ySÀ;¿B$g¾UÀ<õ²6ci@!Cš
,Õ?ýåù×ÇÓ?ÅxÀƄ3V¿¨ŽïÇx¥?äòÂàdÚ?üê#!BE?ð?àØ ÀaŠ¿ÃSGOÊÄ¿çñ-Õ%`ã¿á…\–$?Ä?ՂþÍ{AGNbcuFIRST J130948.8+371651?ïþ"p'?2ü§_ó?/v¸ÿÞ¼?2ü§`>?ïñšïP±?ƒ²kÉý:?\Ê!^ÅÃ?ƒ²kÉý<?ï¢ÿëÇ\å?"Höëëb?‡@(Æy?"Höëëc?ï•ò»—@?ëMýv›?ŸmA¨ò?ëMýv›4FGL J1309.7+1153?ä­ýJÅÔê@R‹">iƒÀ9ÉQì[ÞMÀ<J@~uPå@-Øjå§@%ð|Õ=µ?µ ÏXmTl?¯S"'Û9?÷–…³2ÇÓ?ÿÄ¢–?è*·c®ü¿¬À=àÇg¿ãshãh­¿á'­Ãó	¿ç¥¹Þ²§¿ên¹PïÝAGNbll3FGL J1309.5+11544C +12.46?ïؑÑƟ?ˆ'ô̜ÝT?íÅÇ,/?ˆ'ô̜ÝS?îJ5U?½¡‹Gžö?¯{\¯º®?½¡‹Gžö?;/é?"ԗᇶ÷?œlN¸šç?"ԗᇶø?çÃtk>öq?³Õ/ EÔ?Ðy)'?³Õ/ EÔ4FGL J1310.2-1158¿æ/š½¡g³@IPØ]ú‡À:KÏknÀ<UBí»YÞ@ˆ_X@$(ƒ¬ÈK?¶þ"n\T?'¦Ø؄ø?Ýô^´kW?þ&'Ë¢¿ï(,ÚSž
?åzVs'¿âœ°ožôL¿ãdT"—½¿Þ¤‰ôaf¿Ó°
ĎºÃAGNbll3FGL J1310.2-1159TXS 1307-117?ïÊ~"±?uÍ(¿ñ ?zÀ¿nö§z?uÍ(¿ñ ?ïòÿëøS»?tüO>O'v?Z(XŠ?tüO>O'x?ï"v£°0?…ýÁâ'à?‹"WÜ3Ú?…ýÁâ'à?ï0Ǟºu?‡€U¼uõ¹?™ç'¨±_?‡€U¼uõº4FGL J1310.5+3221¿äôŸÐ†È@TÕ=1¹¶pÀ8M_ŠªŽÀ;[ß-ø`Ï@³±_^	v@eÊål?¤6NàQ¨®?«DTÚ<L@`ù£v'@LVjoàc?ï%tc+Y¿ãE& RÆK¿äe·]®1¿äF'ÌÍ£Œ¿ç™!ú{²¿éécÜHkAGNfsrq3FGL J1310.6+3222OP 313?ïöIßyM?PºOÂoø?SlAÅ
gb?PºOÂoø?ïøË.-Gd?aºg†jG?LÓGJâl'?aºg†jA?ï|ßo?•'SGј?ŸÐ}ä'6?•'SGÑš?ïíû![~?X°Ò¸Íp?bÞ¤æÀ?X°Ò¸Íp4FGL J1310.6+2449?î3*¿Ö@UG"…]¢sÀ:Œ—f¹rÀ<'Ã}˜²@ₓî‰á@o–Aö?»¯£½ú¿¥Ù«#ýÀ?ëᣦÙô@SqîYåO¿äêê>͛)¿Üº[_L¿ÛâCV–æ¿×¼Ù¥"cØ¿ì³+ ?:¨?Öôû?&£AGNbll3FGL J1310.6+2446CRATES J131038.52+244822.1?ïÉ~¥S‡j?v9ÎçžÓ?{@­V<J?v9ÎçžÕ?ïï›ùr/°?|NŽŒtL?`dÐPa?|NŽŒtL?îß¹¯_E?šE
CeÔm?£Æe
­?šE
CeÔm?ï(tËt€ä?Œmê«¡•ó?šñf'oã«?Œmê«¡•ó4FGL J1310.7-5553¿ã_í¨wzã@ˆ.¢ªºSÀ9§¢KïÃÀ;m$²>¬@B;䲝@SsD›:"?ÑqÉ—ïu?Ør­™+@Q˜ÿ?æ @o¦èa¨¼¿àïG€È|¿é'5deÛ&¿å)™—Ž¿ëüXáB¥—¿î¢‰,d?":#«š'AGNbcuPMN J1310-5552?ïÍùՂ=É?~"JGs*?y>á{?~"JGs)?ïù¾§j‡×?h…¸Ïó¸"?IbUà¡Æ?h…¸Ïó¸?êå
Î?ª¹`Fza?ÄkËôǛä?ª¹`Fz`?ïøŽÓKÞ?@Oª>´Ù?MIJЇ¯@?@Oª>´Ý4FGL J1310.9+5514¿åGÞ&`È@NÔ
9À:[FóÚWÐÀ<´Näi¡"@˜GŠ®X@ÅP^½$¹?¸ÒK¼ÁçÁ?§gƒò¾N?êwAë\ÚÌ@ý;Qå¥â¿´XÿJ£gN¿åÓLãÞaJ¿åœ³"íbo¿åöØ9¦ë¿é¥ÖÏÛ¿ïýO¶÷xrAGNfsrq3FGL J1310.7+5515TXS 1308+554?ïòÊñÍ?UÉC­jß}?ZkÊâd_?UÉC­jß{?ïü§Iu?MH£q€â©?:Ǎ´W?MH£q€â·?ïÝ*7؊±?wùû<Åq?qj产Ñ?wùû<Åm?ïÇÇá<æT?j2aþÛx?|aŒÖ?j2aþÛx4FGL J1311.0+0034?í'WüL'@OƒqC9:´À:&­~Rì6À<Ìóc9‹@ Þ.Iš@þM œÃ?·ó;K…w¿¢!¹€Yé?éß[zz¢@7Œnbß¿âEU	FП¿×Oê£øBF¿ã{E†S¿àîÿA"¿ÜÓÄãŸL¿ÙT—¼Ÿ®AGNbll3FGL J1311.0+0036RX J1311.1+0035?ïÛM»K?jph)Ýž?rvðY"Z"?jph)Ý¡?ïûŒ®~Á?V…ŠB=™4?CÍÍFù"?V…ŠB=™3?ïƽ¤@û¬?}81ϐ‹{?|¡-߂)ô?}81ϐ‹t?ï°|ÎÝ1j?p˜Ûæꑑ?ƒàÌH³¥ß?p˜Ûæꑓ4FGL J1311.0+3233¿ÔÂú«.y'@TÆå6P&À9Ú J"cÀ;{Ø=CWn@®´2ø@.‡$L£?ÁÍÊùõ÷?ÐÖ\˜‡K@3Š™K–@IVå¿âÙ¿ë–ñÿ6V~¿¶ªåò7Àa¿ã,iöZe¿ã9ŠÀÏ6¿écÞAp ¿èØJCðð™AGNfsrqRX J131058.8+323335?ìÞ§÷Ô"?³Úóå‹>?¹
ÇxA^ö?³Úóå‹??ïüƒ4wq?Oï5DGþ°?;æ\Güyo?Oï5DGþ—?çø™HöT?°Äíž?ÐÍnüX?°Äí?ïѓ£ó?jÈåW½ñ?w6wò.ð?jÈåW½ñ4FGL J1311.8+3954?ã>c²´@S"Ú<÷À;‹ì §ªÔÀ<ñ令ß@ œÜl'¡?þɋϬ{?οUÀÑÁÔ?«fÝћ¿?àóîå%‰'?ýùö{œÙ?ïý'w>$ÿ?À7`"j[¿è™â"µ.K¿Õ4¸#G'Ë¿Ö<‹Á¿¨w¿äðÖÍÏ3AGNbllFIRST J131146.0+395317?ïþPíæ>?1[t…Ã?*ñ!žœ/i?1[t…×?ïøJŒtau?r,oÖµ_?NÕÎ.z+W?r,oÖµ_?ï܈ÓåҊ?vDڙ¢]?q»–
»??vDڙ¢]#?ï‹UZŒ?y /Ü¡	?*©\ܹq?y /Ü¡4FGL J1311.8+2057¿Í?Ò9‰`B@T'(ÂzÀ:³ŒbÀ<k]Îpk@±ObhÕ×@
aûc?Åù‡€gny¿Àkí"ì±?ú
Â*²[1@"Àl—¿¼ Ì"Áé¿í66Œs¿ì£ÙŽ|/&?ºÕÊÍC?¿ïÿöùŠp?ì:G#ªÿóAGNbcuMG2 J131144+2052?ïۈmvµà?€ÃŽœö ?r;ÉD¥P?€ÃŽœö ?îÆ5²Z×í?¼¼lRÆÌ?£œ¤ÚRA?¼¼lRÆË?ï6ÔdVܸ?'‹ÉJïh?™%su$i&?'‹ÉJïh?ï"u§.%á?ŽƒZBJD?Šâ–4v‡¢?ŽƒZBJB4FGL J1312.4-2156?¶‹=áZˆ'@DUóFí$À8µÁÉc‹ÁÀ;¥'õÉE@ýêAÞG?ý:61ë5?¨ŸCãÀÀ`?Ãc>Ò£¦@Ò­`ûH@¥ŠFjr¿áËOK¿ÍÐ-hî׿۠¾øN¿Ý^{ ۑ¿å«(m"˜¿êIÈ ÈdAGNbll3FGL J1312.5-2155PKS 1309-216?ïÓÃç	è?vw¤Çk¡?v{z?vw¤Çk¡?ïë 2£^4?|?÷?év?dßÍ\¡ËÂ?|?÷?év?îãcѝZù?š+§ËL^?¡ÉÂæ*Pl?š+§ËL_?ïÂs-kh<?jv{.o?~ÆiJKâ?jv{.k4FGL J1312.6-1900¿ÙSR¯®@EÈÿ%¿­À:ê ú¶ëÀ<|K2-y¶@ …½ôAÛÃ?ÿ}"jŽ?©Â܉s?"†_ޕ·?ÅõÛĈ?ÿBX•~Í¿ë‡e_L—?ïóÜÁ6–•¿ÚÙ]ÔÇm¿áőڈw2¿ä†'ø»h?º)WgEžAGNbcuNVSS J131234-185902?ïû9SÀ?<%í¡E=Ë?Cú±È?<%í¡E=Ô?ïúxsù†?^ÿ­ü=ý¨?FŠ0ëµ?^ÿ­ü=ý•?ïâóªËêá?s±áÏé(È?mU4¯?s±áÏé(Ë?ïžp$à…L?wÓn¬÷u?ˆcöÇÞ¬À?wÓn¬÷t4FGL J1312.6+4828?Üð:@QÔªà"À8‹p*ÖmÀ;ÊPSÕj*@²6¡&Ö®@‡¤WÙÜ?¡HÔ|ì™?¯¾"¤9I@>vû	@ R3€5¿µùN`
VÆ¿ÜÆày§â¿ã%p'Iü¿áW^‹¦'¿æàTÔmªþ¿ß—ô}ë¾*AGNbcu3FGL J1312.7+4828GB 1310+487?ïý¡¯ñ«­?2Tõ)³£^?2ò€r¢'E?2Tõ)³£\?ïûLÖï#?VÐG‹ý'?B̧Cv
?VÐG‹ýy?ïÓEX?{X<è¶aZ?vuÝ~Ô‹?{X<è¶a`?ïÿþ»ÒÙ>£=z]ÅÂx>¦ôBÒp?>£=z]ÅYë4FGL J1312.8-2350?Χ(x,œ)@Caÿ.Hè§À9»¤ûÍkXÀ<*b{ö@ 7™Ig¨?ûîPrß?¸ž·¥+?·í§¸Á''@eÂÒxy@Poĉy?í¾aÔU¿àR*ڟg¿Í'&]·Á¿ÞÅå"S·¿Ò‰ÎÒ`‹¿âÍ
>××AGNbll3FGL J1312.7-2349NVSS J131248-235046?ïæ´vÞÿ?aѨšAú?iK‰â!ž?aѨšAú?ïð ¯À½®?q"f¹Ûb?^¾ ~"¥Ù?q"f¹Û`?ï­Úœ/h?"?ú‹se|?"‰Xô8eø?"?ú‹seu?î¶Äpá<—?‰Ÿ•e+?¤"¸ñì6š?‰Ÿ•e+	4FGL J1312.8-0425?ÜúÉÐmð³@MÜð0$À8åö1J%À;߬ÂkJ@ŽØ™´œ@¤u_þmY?¬wìÃÂ¥?Å'Øa*'P@[oŸË@hJã©K?臕ÀÇ
¿ÛAGÞeü^¿å¨ïbxñ¿ç¸Ž·«¿ç'£²ø¿ïÿK§ž?AGNfsrq3FGL J1312.8-0424PKS B1310-041?ïïN= Ü?]Ž˜ §_?`±Â_#î?]Ž˜ §f?ïô³¹_•¯?kµ,`â(?V˜@Ô !?kµ,`â,?îþ›¸™â?–)Æc›')? D6aÚ?–)Æc›'/?ïüz|ƒoç?+˜7T®§?<,ä€Ç'?+˜7T®†4FGL J1314.7+2348¿ÚXò‰Ò
þ@Tò	ª£­À9;Ñ|^öÀ;åw¹u4@dçv¯Š?þV½+o"?®t*a"ð?¸ÉÏAq9~@HŸ¬R@€\óvè?ïf* ºà'¿ßhøÑî¿Ý¡¼þ£‰‡¿à˜B"пâúK '\9¿íÍ;5À¬AGNbll3FGL J1314.8+2349TXS 1312+240?ïü76e¦?5ØHe!ç?>FKÒÑÇ?5ØHe!(?ïòi.Šúq?mÈçýø$Ù?[-¢ê 1?mÈçýø$Ý?–…X?ŒÜ²â'Ü—?ŽÖZ\ª\?ŒÜ²â'ܝ?ï
}x¯j?ƒä>(¡f?ž°Pê¿E?ƒä>(¡g4FGL J1315.0-4236?îcÝbsvW@4O~ÃT~À:&¤/õ'À</ßÅoá@"`3F~j?ùÿJH"®?Á5Yh§m?¥$Y%¶?çoPð³[â@̪7Ìu¿ïù>Ú[V?îÉCu –
¿æMà}ٟ™¿ÖëDÜþÉ¿ÇÃdCK"8¿ÖA_›ÆðjAGNbll3FGL J1314.7-4237MS 13121-4221?ïù#"=_ò?IvÑ{™à?Ksw
€9?IvÑ{™¿?ïö¡ÏtD®?r­9
°?R¼av¤—?r­9
¯?ïÆLîÚ["?7j_òw=?|و'Òo?7j_òw;?ïžàËù9M?z—uºÒmž?ˆGͱ¬Ü?z—uºÒmŸ4FGL J1315.1-5333?ÈÆ&Jº½q@"HϧÆÀ8¦m¢šÊÀ;RáNd"@Ù{Üpê@‡½#â]?«AÔ&?À^GG@֜¾H'@÷¶p"è…¿Ñ慛
¿à†Àyt¿åUD€ª³¿æ(°B¨q#¿éh‹¬"q¿ê_Sb'½^AGNbll3FGL J1315.1-5329PMN J1315-5334?ïäç«i{?n»Úq@s?kâT–…$?n»Úq@w?ïõë;Wî?p'Œ÷/?UÔ)‰P#?p'Œ÷+?ï"³§?ŠHº14&?Žþx"?ŠHº14&	?ïüW}T$?-mçú?=C^Ú¢?-mçú¾4FGL J1315.4+8453¿ï772#ڇ@@?·¥ôÀ:ØÙ.IÀ<jÑâ¶C@xIéW@"}€^_1?Æ:azÄAc¿ŸÜŠľ?׳Ûåž@–ŠýtŠk¿×V^?&¿ëpBRŠçO¿â©å‡ó¿çÁ½ªE
¿ïÕ@%Nn¿í€MÍé,AGNbcu6C B132240+850531?ïñTg7\ƒ?r±ùgEà?]W1'FúÞ?r±ùgEß?ïö"œoa§?w~ň¦B?RöÇ!<²?w~ň¦B?ï…äÂýŸÁ?‹˜c"'su?Ž†Ï@˜ï?‹˜c"'sr?ïÔW­GŒ$?d.]‰²?uÔ)\9ír?d.]‰®4FGL J1315.5+1135¿ëKê¼0Tž@R]­BÃÉïÀ:" Rñ?À<eïÎY"Ç@ îRî'?øú™ú©v?É#–=áã?ËÐá.ƒ¡
@7°pu³á@Ôüj?ï)³ʅu¿í¹´V´A¼?Ì´ÆÆ£gú¿¿›Gn©€í¿×{°&äp¿äÎK^˜AGNbll3FGL J1315.4+11301RXS J131531.9+113327?ïõHÜ:Ì?U"s:f`?UnGŠgÌj?U"s:fc?ïú§¬ù@0?X>ëh{¼?EaLÿ@n?X>ëh{·?ï¢!&àù(?""†óX
?‡w¶GÁµÉ?""†óX	?ﯮǴ@‡?r۔8^Ë?"NïÞ+?r۔8^Ë4FGL J1315.9-0732?é"Ûƒ@ñ:@Ki"}ŠÀ:
뱔b"À<(^Ì>1"@ƒkµ/Í"?üO9#7=?¹…cÂD¯?Á·uø®@.d²1@@mdDM6ê¿Ü$´?b@'¿Ù²ÕÎÂE¿¨ˆÕü÷7¿ã!¡ŸØx¿Ýa'nê¿ãwקò"AGNbll3FGL J1315.7-0732NVSS J131552-073301?ïúFÀCÀ?aápUæë?Fäý¾ñp?aápUæè?ïü(™–S–?\æÛq½?>»3McO»?\æÛqÃ?ï©ÿOí¯?"bÓ6ŝG?…€;ì"ó?"bÓ6ŝB?ïú{öý߶?2æô"Ì?F$(T?2æô"4FGL J1315.9-6349c¿ãì:¾k] ¿ña၏·™À9ªl…dXoÀ:²/€ KÐ@'±…"@šTÅT2‡?Ò§9)í9T?ºM6iž2?äkž´‹g@T,Ž~]~¿ïüœž0Ø?îï7œ¿âöÙÑ.[¿â©‡¸Æ…‹¿éUDÀyWZ¿ïðdìé¢ÆAGNbcuPMN J1315-63540?ê=RçÙ;(?Æúö‰‹óÝ?Ç
´`›\?Æúö‰‹óÞ?êì¼m™>?Ò½ó"·zk?ÄOåI›?Ò½ó"·zk?åþ»bÔÔ?¼°—ÈXö"?Õâ‰:VY?¼°—ÈXö"?í§ïÜ	R<?¤Nç°0r?²Àµn+?¤Nç°0q4FGL J1316.1-3338?ãY}8ä-@<ôFs×ÜÀ8gõò`MÀ;ˆÏ×CHT@Ÿ­"Þ@GØåó?¡õ'	^Ú?²˜Pï0Ï×@c3á®Ü!@…Våb¿ÐÒ¸©)¿ÝÖ¾=<÷W¿å3¥´Z@¿å¼ä!}(J¿åUK Â€¿åZ‡5DAGNfsrq3FGL J1316.0-3338PKS 1313-333?ïû¨L²°†?=¨+•¨N?A^Í5=ël?=¨+•¨u?ïûr!†ï?`Q{þçà	?Cº7yäGè?`Q{þçà?ï°½/?€ýô͙"ê?~÷§¡véz?€ýô͙"è?ïÿš‡fé>þ4Y¾jÑ?	~^&EÃc>þ4Y¾j%4FGL J1316.5+3013?㩏PñiÄ@TëQÕQ×À;¬ˆô'À<ÿé]&KÄ@e°ŸÅ'¬?ûÒÂÊëK=?âÀžìå?қ‹vÁ'}?ö;¥wô-d?þ•ùqE'†¿ïý.)7?ïÄҗç貿ìV́¨Œ&?Ӑ¨"C3¿çZüۈQs¿ïÿ^Ô÷"AGNbcuRX J1316.9+3014?ïóXÄ>?fu`Ɍ‰¯?YNÅÞw‡7?fu`Ɍ‰¯?ïéâ§d¡?"qcT?P?fóX›_9?"qcT?Q?ï[ÕïÌ)ß?= *«jf?"…BzÄ?= *«jk?ïf¹'¢­ª?ˆ¾fcþ?"(Í«ªJ¾?ˆ¾fcþ4FGL J1317.1+6613?ë'ëò…–@IYÝDUGÀ;D·éæ¹À<ÑÜKÅÑ0@ƒÁRñ©@|l—ØÏ:?ÂFµœ¬2¿§¨¥ûý'ç?âN¢?Zˆã@ÚýA‰¸%?î†@áDž»¿âk
ÀMb‰¿ê

Dý`¿êjˆ¿¬¨À¿ÝAÞò"2?r<TçZdAGNbcuTXS 1316+665?ïìEôyE­?cWÌAKH?cº†ºR¹?cWÌAKH?ïú$ç$'?fƒ«lÅË?Glc—m¹'?fƒ«lÅË?ï‡Üº#Y_?†îq'ì?ŽÑw)¨<?†îq'í?ïâÎ
ãpå?_c÷ø1ßp?m1õ%?_c÷ø1ßk4FGL J1317.6+3428?å`ó}ÅA@T0Åë1;âÀ9ʵ™ª`'À<jz4y"P@yáäáìo@÷
=p£×?´Qbޜƒ?´Ñ^¬ÞšÖ?üëNbc¢g@Vð|ªK¿Æ!Ï4`¿å};?HÜ¿æÔXÖZë¿å¡ŽàØóL¿í+™
þ`Ä¿ïâfê%xAGNfsrq3FGL J1317.8+3429S4 1315+34?ïûôú8® ?7m폞?@,Ey­?7míW?ïüž^paŽ?QE¯‹Šg?;
|ó"R?QE¯‹ŠY?ïä4;cw?fn¶ ÕÌ?kˀĜ‡à?fn¶ Õ¨?ïúÇñ];â?85.´Çü\?Dà:‹wy?85.´Çü]4FGL J1317.6+7450?Ԍ°ûf@E<³åuÀ;'mÄÿxòÀ=ŽVox^@W"f1bN@_^4h½?ÏÇíÕ[È?Æ(t"OÓ}?íëù¸¾"?÷õ±Ím¿±â˼¬n3?à:õ¿ÏÖ"î9.¿ä©L•£¿çë@àðÆ&¿Ó~/?‰AGNbcu6C B131714.7+750402?g9Þd?c'îp©?S¦1ˆg?c'îp©?ï¯d­Ž4"?•Q!óÎݾ?"&ԜrÛ[?•Q!óÎݾ?îå±2O1Ê?•
qx»K:?¡¤ìÛãk?•
qx»K:?íü¼?šä5ä—?´€éê?šä5䗁4FGL J1318.1-1740¿ä=dS¾ës@F]6Þ¹^[À:º¸ÌdÈÀ<fèQ'N@ìË]ë@þÑa‡•?È~ÓD¶?·—
ž¦Ñ?í;Ì^èã@¡ Lü‡û¿ê=G‰+M?ïëÒá长êÀ|1¿Þ¼ŒxHæú¿å)+<Ĭm¿ïÿóÖ&ãAGNbcuAT20G J131808-173536?ïëê%sÇè?søú÷ý?dڌ8´?søú÷ü?ïù§²2™¶?ej3A"LÏ?Ia75™"¥?ej3A"LÑ?ï›å¨`ü*?‡r?'œ?‰•çÀö?‡r?'œ?­8Ž?z¬à0ŒFl?‰'Ô±Ü~u?z¬à0ŒFl4FGL J1318.2+6754?î½úûëõ¦@H±Ù+áÀ:âñ#ôÒÀ<ö1ø .@ʁðÛtÛ@"d¼B;?Ä+þNå?Ê'€EŠ¤@aãðÕÁ@Ÿ
qÈð¿Þ˜L<™Ž\¿ÑëŠ<¯]Ñ¿äiü¾, ¿Ùº?–më¿ìE ž²´¿ðAGNbcu87GB 131701.6+681031?ïüÁ´î–?;1ý¸K£%??)òX‹MØ?;1ý¸K£S?ïüD¦v
ò?VB|åëÓ?=ÚÌO¨l
?VB|åëÇ?î¹mUF9E?˜‡Z^óÇ?¤i*«œk²?˜‡Z^óÈ?ïüÈÀ?,Sž¯`?;¹ÿÇvf?,Sž¯¡4FGL J1318.7-1234?䆈jÌф@HÞÆÞvB|À9ÏhµËÿGÀ<BÛ·K[H@Õ'*g@'Ú˜gjr?µ¡N›Ä?²²Z@úW[?ühMÇ3/Ø@©vƒ¿èŽ?ïûv=žñó¿ß%ôñ¯e¿ãÚüȼ¿á{lB†Ï¿áÈJÕ¿ìQ›žV—¼AGNbcu3FGL J1318.7-1232PMN J1318-1235?ïûHÍbKï??ìv¹Fۖ?BÜÊvÐCf??ìv¹Fۇ?ïø\âÔèä?bcÁŽ«c»?NŒt¬\qô?bcÁŽ«c¸?ïé40¯TB?lR¤ßJ
Ä?fËÏP«¼f?lR¤ßJ
µ?ï—Ò~JKg?q[¾ÅðÊ¿?Š`mm&N?q[¾ÅðÊ¿4FGL J1319.5-0045¿í҈äXЗ@N¦ùü°À'À:nd-§8À<lf/	@ؼKV@G@ÿ¤?»L·Ñ=ö¿‰ò'­gë?ÍåÑ*ªx@i?%3?ïü¹>z¿äAèÜy¿æŒížÔký¿áXl"h	Õ¿ïü#!BDô¿ë‡ù(ujAGNbcuPKS B1317-005?ïù<-¬»d?beÀqº¥×?KIMo?beÀqº¥×?ïý*uÛ»?K°•¶?6¬W".Ž?K°•£?ï×@6%Չ?x"`sZÓu?t_äí;²?x"`sZÓe?ïô¦U"^?HÚ-FuU?V³ÇU»AÔ?HÚ-FuW4FGL J1319.5+1404¿Ù=?ʉþ©@RؒyèÀ:Ó!ž¶9À<™>ÔI™@øËagÏ?û߶må·?Ïâ+™5ñ?ÐA´ †å@¹	k¹Œ~@v®óH?é¬
¥0ç¿èæä:§›»¿­÷Àkj‡2¿á(ŠÎ$»¡¿Õ/æ5T¿ðAGNbll3FGL J1319.3+1402RX J1319.4+1405?ïû˜²¥–?@fwǎï?A5kí¦r?@fwǎê?ïû¡Î†%
?V%)Š?AxÅçkÏ®?V%)Š?p³"F?‡íA^â{?Œ"£ÓîB?‡íA^âz?ï›%ÿ"Ô?u¿ù£F÷?‰6€7~
Á?u¿ù£Fî4FGL J1319.8+7759¿´Áç(Åã@C"{¢7ÍÍÀ:)6&,ºÀ<ªÖR5W@¾Ë$V ž@Y©qÛ?²"`_;Ná?Spaù.@
‹éû†Éˆ¿åÐ!ÙC©¿Îd"i®ðC¿ä΋魮$¿àU<þ
6Ÿ¿ßÐ`zn±¿Ö Uu}ZŸAGNbll3FGL J1319.6+7759NVSS J131921+775823?ïý,q}-Î?1ïÀÄͦ7?6œt'Œ}?1ïÀÄͦi?ïýÞ-oÂ?H"œ–?1n"ø(?H"œ†?ïñßoDÁQ?hY`0=€6?\A!v}^v?hY`0=€.?ïýCÅä
?&nþÉnÃ?5áÐ߯øÓ?&nþÉn×4FGL J1320.7+3314¿ï™Ìðp±@TM*®)s—À:ÖÛÃ	ÕlÀ<€ëLê"@êØ¿IV‹@g†
¢?Íía—ÊŒ?Ò±×~¶ß?ÿi±Y©¿'@(¡ ¤$ã?ì†X>…vÍ¿åÎj[¾l¸¿å­u"›Y¿ëÞ`]Ï·¿àù«ƒ¿ïÿÒþÀùAGNfsrq87GB 131814.4+332742?ïø¸A_$?NêD
æÔy?Múƒço«?NêD
æԘ?ïü˜€•ÏÊ?P6q*Ùsr?;;ûQ­i?P6q*Ùs~?îÏÒ:½õ?–'';bn?£Ü_ä ±?–'';bo?ïÚ+½!íL?d1†|cO?rê!o	Z'?d1†|cL4FGL J1321.1+2216?çÈÞ¼L@Tlºˆ&«À8ŽÅâÍÀÀ;°…ù©¤ª@ï°¨ÔÊó@@gc¼gû?¤)0N&v?³Ú6lΊg@Î^'lVj@rø_¢¨¿ÕÚj$"¿àđ"èYñ¿åG˜_ݶ)¿åž@ÈG,¿èÞê¦ÒgA¿ìJˆ_	¥ÆAGNfsrq3FGL J1321.0+2215TXS 1318+225?ïø#[â­¸?DsüԊâ(?OruIï?DsüԊâ0?ïûv¯c¿Á?TGõãÿw?B%Bqø)?TGõãÿo?ï¿åÒQ˜ì?~`®Y·$t?€‹k™Åp?~`®Y·$t?ïüÙáær¦?+ŒËg	‡?90ðÌjä ?+ŒËg	s4FGL J1321.3-2641¿ï±.µT@AØàÉÙÓFÀ:ب)À<L[œÞÈx@bó•8Œ@;þ¦c¬x?ÀªãƒrÁ¿¶B³-êI
?öª¼¤¡5@Tä©~>¿Ï""ÜÉ9¿é1àþ¿ì'ð}V¿ŸPg˜âÜÑ¿ç ÕÍýNu¿ï÷ŞÛ!úAGNfsrqPKS 1318-263?ïîFÆg?a¤?"mµ?aä¹9˜r¬?a¤?"m«?ïæXỸ?•ù.-¯õ)?i§¦3|î?•ù.-¯õ)?ïüfw?"8Ïãþ"»?‹ÀûxfaÌ?"8Ïãþ"»?ïÀ䮬Ê?sd›»?ž-¨©š'?sd›»Ÿ4FGL J1321.9+3219¿è–"t²OŸ@Teˆ±Ù+À;IÀÜԁÍÀ<¸Hi%]ˆ@»Fc'ŸÐ@À
¼%/?Ål¡«¶Ó¿–[߂d§R?ÔÌÎzKö@ä*m'ÓÒ¿åV…þ\;ë¿äæœau÷¿çSˆ]‡º¿ÝVÀ	¿æ\C'‹¶?‹›Q:ìKAGNbllNVSS J132159+321903?ïû'«Wh€?:ììX6
¦?AõR¢]üE?:ììX6
'?ïý›ätÇ?MC×i*T?3' ÜYÖO?MC×i*^?ïø*L?—ý?X¥ù³à?OVÏ 3?X¥ù³å?ïøvløYâ?A+N2æ?N&L˜v›?A+N2á4FGL J1322.0+8317¿é<aÖ±
:@@ã×<'W†À:\Û¦"c§À<@–ÉÁ@!š…Ò½R@èJה§?Á<´ÿ?Á¾z¤‹åý?üà·õ¥3@Á?à뒶?ã;xçrj¿Û®qÊG·¿æžÍë°½£¿àÁJ³οëù®AÇJ­¿ïýR†Q¾AGNfsrq3FGL J1321.7+8312S5 1322+83?ïð"$Í>ƒ?YÍ/Shhf?_»¶e'õK?YÍ/Shhg?ïý"çÿâ?PO÷Mñã­?6èÀïO,?PO÷Mñã¹?ï¢ûøÄYï?…KŽÓ©)?‡AÎé"{?…KŽÓ©&?ïûhQã?0òñk.?B^¸õøzS?0òñk74FGL J1322.2+0842?åðނn'@QŒ2 f<uÀ:gég7F¾À<~ˆA'O@k‡}'@_`'÷–¥?¾&4ÈÂÇ¿—©Ä—ÌÝ?Ú5˜}ºÀÜ@"{½™Á¿Ú¯Þ|·â¿ç–œŸ2ŠÂ¿â.5!õÉ¿Û:…M\T¿ìrH½3«¿Õ±$ûŒÿAGNfsrq3FGL J1322.3+0839NVSS J132210+084231?ïöÐü		F?Háðùºü?R^ííté?Háðùºé?ïýæ¯T<Þ?Gç#áÂ?0ʅ^3?Gç#áÂ.?ï©exé?ˆTƒ¼œÿ?…¦¡Å¹:?ˆTƒ¼œÿ?ïü)´—i"?0È¡/Ið?>²[D¶ðP?0È¡/I.4FGL J1322.3-0606¿ë_×BÞÚ@K÷²VÿÁÀ:óY'BCÀ<´¡õˆ­¹@@ ?û4ï*Ŧh?ɂ§Í"]?Ö¨B¿BJ¨@3å	Út?ÿl¿y'3¿ïÿúVrÓ\?ïÿêњ'ç¿Ô	B%¿ÝjwØ~±·¿âYDàá6¿ïý'Æf>AGNbcuAT20G J132219-060619?îÎù^¢$?¥¢JÎöò?£jݾ©?¥¢JÎöò?í¥~Ïz¨«?À©ÍA?²Ô	"*º©?À©ÍA?æâþ_fuô?·ç—˜2ÀÆ?Ò:A3?·ç—˜2ÀÆ?åÒu¯¤lî?´gP\ô??Ô[ ·&$?´gP\ô@4FGL J1322.6-0936?¸gûíÔf@J?^g"dÀ9.ø6#
À<"*M±c»@SoЍ@'êÓ²š?­Š¿q6	?¹¸A¿+é,@û#š8ûÊ@«AOÝ8¿´"ôxA¿ã¦¡Ÿ¢r0¿é,.âkšƒ¿éŸÎ!5¯º¿ç4R¿æ@Î&i UAGNfsrq3FGL J1322.8-0938PKS B1319-093?ïþœag¯£?!÷hÜJŸø?&9é…¿ô?!÷hÜJŸµ?ïûÕ(Ë>?Xã'ѤA?@«\Óïj?Xã'ѤH?ﶱ;'?€ôZ~o÷î?'S±;¹[·?€ôZ~o÷ð?ïÿ‡a?âD?ÈÒr8=?'°nÍ?ÈÒr8<q4FGL J1322.6-1418?ïÝTo}"Ê@Gð*#¿ø©À;wëÒK'ÏÀ<°$?ziS@ d°êöY?ÿ)¸`.>?ÑÔȄ=¼Ï?Å´!ZBÁœ?õGuàVíM?ôí¡
Ò
¿ït†ŸÁÑÇ?ïüÖ 
L	¿âL€ Ì©;¿Ý3<mn˜¿äô'Þ½¿âÍÐØËÑAGNbcuTXS 1319-140?ïø¼Ðí·?T
tÛ±?M¿"I$Š?T
tÛ±?î‹n›Ÿ¤ ?·Bwñ¼«`?§IF¶?·Bwñ¼«`?ï°2˜ø×?ƒ5ò•èâ?ƒóYÁÿÊ?ƒ5ò•èä?êÍ®Ì}¤{?­ŽHÑë;?ÄÉDÎ	n?­ŽHÑë<4FGL J1322.6-1617?íL%$K`4@FöFñVÀ:½i&4G/À<€SM"î@FÒ̖5?ÿ~"ÐÜý?ËÈÕFmø?»@ö•H&4?ñ%HĔïç@QÉc?ïñÑ~N³¿é§ùä]K¿à/÷¤ç«¿Ödf[ÿ…1¿ãðý=ØӖ¿ïÿøãúAGNbcu3FGL J1322.6-1619PMN J1322-1617?ïÿ5ó*?´¤ð¯å2?_¹AšÚÙ?´¤ð¯åg?ïúhº~¶?]ㄻýÝ?F]%¼ß?]ㄻýØ?ïí÷+q'~?fC(ë%Æ?bԎ}ƒN?fC(ë%¤?ï‡É½mÿç?sjÆ~º¾?Ž
¤€…?sjÆ~º¿4FGL J1322.9+0437¿æQ7† <@P'ò{xÀ:ïùwO¶À<™€TN5î@ L—ú³?ùnˆwÆ?ÔCÔýKp?ה&}˜1:@2äÄ:W@ʨ<ʋª?îÜEæ"0¿ìõ΃†1Þ?Ïb`\â@¿ÂôƒJ!â(¿æ5'ST:ë¿ïñH­ûŸAGNbll3FGL J1322.9+0435RBS 1257?ïüýº#oz?9ycŒ?8.ä"/Æ?9ycŽ?ïú±7à¸?[õÃå?E; i?[õÃö?ïÁSòHԗ?[Lâ..?Vە´B?[Lâ..?ïi
š÷à?}ѹdÓ>?'Þ¬¡Ãö?}ѹdÓ>4FGL J1323.0+2941?'à}ÅT@T¦}¿H€À8è[;ùÀ<ʍWkø@9Dü3l¿@êKáQ?¤p½¾x1{?«²DœxWf@œÄÇDÎ@º`@²w·?Ç2"åX¿ßð(‡ƞ¿ã½†]ҙ¿áŒé½ž[ ¿å>¨²;Q¿åwR|¤–MAGNbcu3FGL J1323.0+29424C +29.48?ïØ­z'?˜JVÁe!'?ÄêN®?˜JVÁe!'?ê'Œ
¾?Òðy[ž?ÇaÏՋ­?Òðy[ž?íVÁÔnË?£ü$p"V ?µOañ\‰ª?£ü$p"V ?âZä "i?½Uax`?ÛKö7¾×.?½Uax`4FGL J1323.9+1405¿¼wóûá˜@Rº×à&EåÀ9æO"}ŠÀ<3PëªÞe@ cøÍܗ?û9AŸÝ€y?¾ÏiŠ2H}?Á­wÝ\<@í†"ÄP'@¦©øa{?螺¯ÀLŒ¿ä—P~"Ñ¿Þˆ…3[!¿Ïñ[øNZ׿ޠÁÁ€éJ¿æ/RY,AAGNbll3FGL J1323.9+1405RX J1323.9+1406?ïû&Qý_?Dt_¦r"?CÇf¸
€á?Dt_¦r?ïú«
oçù?XÈ_®»~?ESÖ@` (?XÈ_®»}ý?ïÑèZñ:u?{=¶ÿ?w҇bÆ ?{=¶ÿ?ïÆTdõ¿D?c¨'HT-?|Õͅ ]û?c¨'HT+4FGL J1324.0-4330e?Ñ¥\QD\@2ú&€IRÀ7®Í™{f©À:ØÆ;¹²@D*Se­¯@Äw¡!MX?£®¡†­?´-2<@à
quŽ@ô‰PKFû¿Ú=1cÐ4
¿ä+ïý©c'¿ç9m	Ö¶¿çÓÞ¿=˜¿è˜—;ˆ¿ç04{1ÐAGNRDG3FGL J1324.0-4330eCen A Lobes?ìš•fj?»QD"5ï¢?¿k/{TÌ´?»QD"5ï¢?Ø2=¡H?Õ–9˜Z?ãöæát/\?Õ–9˜Z?èr/.åB†?±æ'
¶y?Î7CDjõç?±æ'
¶y?áç†:ì³<?º"ô:ö?Ü0óŠ&™ˆ?º"ô:ö4FGL J1324.9+4748?ç)ê•Ë@Q³AáKàÀ:A(Ñ°aÀ<lÖ#£Â@+»öÀ'@#ˆ?¾äaéÔð]?¬PÑÿ'›?é"x¸xò@aŸ~àÛ¢¿Þ}³¿µ¿èüØÎbÏ¿çtøÀEªÚ¿ç8uý³¦¿î'âJãS!¿ïýNª‡þgAGNfsrqTXS 1322+479?ïþЙ
?!±Ð³è?"öo/θ?!±Ð³èx?ïý¥~¬5?M¡È±‡?7¢Ô
žTE?M¡È±ƒ?ïîû+ö+š?_yš`/?aÔ	ÔfM?_yš`/
?ïþC™\¢?¼";/þ?+Æj>Eä!?¼";04FGL J1325.5-4300¿´ï­Svß@3k8''À7~'æ!1©À;H4[Q_n@@`MȊÉ@:´œT^ý?'œÅ+	¿¨*Àüg£@‡0ž-}@!¯Påö"¿Ñ{%û'2¿çqÊÛ[¿è½*BsÂð¿å½Ž€á¼É¿ã1?=,±9¿ã`Æu(AGNRDG3FGL J1325.4-4301Cen A?ï¬ÜU'þ?">1é¥O?"Èê›Û€>?">1é¥P?×{š¨Åk?ؒæÿ‡
?äB2±+J?ؒæÿ‡
?ìò^qïŒp?¦y"Ô¢º6?¸mpƒœw?¦y"Ô¢º5?܀GÛIÖõ?Àq°¤~:?á¿Ü["?Àq°¤~:4FGL J1325.6-0227?ꊤ]¾€@M¤Ù¾L×IÀ;$­‹¾åƒÀ<¡Š¯@ q‡^Ù8?ýªHiü?йܚ )×?րB¸â4@Á	š³u
@,DeN¿ïþ"ƒÕâö?ïüA™þCg?èFp¢¿ÖµÏÅ¥'¿åˆqy‹¿ï²!…‹ÅœAGNbll1RXS J132542.1-022800?ïÞuÚ?l©ƒl¾RÚ?pý|Eâ?l©ƒl¾RÔ?õ€ÒÊ?¨R"«Ù	?‡ÚŸËMŒ?¨R"«Ù?îë˜"âÏx?–€gžûÝ?¡F}ÑÓˆ?–€gžûÝ?ë*¹-ó$t?¯l/þ1m?ÃUH3n*?¯l/þ1m4FGL J1326.1+1232?æ¿í"Oi@RRwÄ\»ÃÀ;p`B_öáÀ<ÁîqbBë@ ŽG¯—í?ößùµc#¼?⧻Ðüv?×k…òž?ù!¨¬\ý@]cIP€÷?ïé`p¾.¿­Æñv–¿ê˜¶zzða?Àe­™UÑï¿Ó
Ÿk?¿¿ðAGNbllLEDA 1410672?ïõpÞÿƒ?]¸—¶Ç¼û?UÇBûV?]¸—¶Ç¼û?ïûEh֙]?`fð×Q¡@?Bê\¥š†Â?`fð×Q¡B?ïuÖÔHF?Šú"¹»?'E%÷E?Šú"¹¹?ïÂØPmUs?s¤§›û"®?~"×ÉUG>?s¤§›û"¬4FGL J1326.7-0503?Ï?Sá‹þ@LXÅCk›À;ÞÈè;¾À<×ÁЈg@"æt™Z­?ù2Æ[™ƒÊ?××Õ^Á¬]?´ìU~6¼«?Ԟ$ƒBM?ÿŽÞëuj¿äÁ@ýv8¿â¿Ýѿ恽¥œà¿ËbFÇÇÄ¿³ØDЩ*¿ÔLw½PØáAGNfsrqTXS 1324-047?ïþé´ö6?ηôs‡?!o"°œ˜&?ηôso?ïügΘªü?^ªfÊ2Z–?<Á‹:¨V?^ªfÊ2Z?ïòéƒn?f•R"FÖ?Z,ùÉ#ÜÓ?f•R"FÇ?ïõ€ƒÅ?NÖsÁ‡ç?TþùÀuþü?NÖsÁ‡î4FGL J1326.8-5256?ì´óÊz]ÿ@#ÀL‹ÉÍÀ8"¶»éÀ;\hÑz±w@¡×sï»å@mŠaî1¡?©9è?U;­?Á ãd鹘@ÂÍáŸÂ©@ЯE¨UÊ?ãýߔO­½¿ß*ø…«¿â\¾™XV¿äsY(B¿é€ÞLQk¿ì5Þ>XˆAGNbll3FGL J1326.6-5256PMN J1326-5256?ïÑf"p "?pÏO0׺"?wLîÇïµ??pÏO0׺"?ïëÍ4¾˜?]àžžý?dø2ËAgÝ?]àžžø?î—lëZ?›½z4‰†ÿ?¦‰1NŠV"?›½z4‰†ÿ?ïö¼´qAg?Amhö8¸?R†—}3?Amhö8©4FGL J1326.9+2210¿ï½À"jm'@T"¯ÌáłÀ8à~֟´fÀ;ÌËQ¢Š@}YÏT;—@î,ëñ?§›¶Õ>¶I?¾L`RP/@]"Äm'º@¼]*}'¿Áç~~á–¿âYÏ^ø]õ¿æåÂ!M,¯¿æçÁz‰3¿éò¶ÁG³s¿æîè`Q#‰AGNfsrq3FGL J1326.8+2211B2 1324+22?ïø|&"l?GºYYOÏ?MÊe²RÃ?GºYYOÏ"?ïøÙA¼ÈÒ?_kOÆÂ?LšùÜ·Å?_kOÆÂ?ï¶ÐuRö…?€A?O½?'Kâ«B^Ÿ?€A?O¸?ï끙¡4?Tº]&j»?d~f^oËþ?Tº]&j·4FGL J1327.8+2522¿ãì%³¾·@TjGG"#À;¢
6Ih)À<ÜS'ˆ@!S `Q®?÷_›ªcì?Ú±ÜÜdok?Äß	$ìÉl?æè$¬‡²ç@ßbݚÐP¿åJ›ÏÔ¿
¿ïÔ~ýŒ`?ì?©-‹S†¿ß7ÀÜ~œ?"?QyšJÄ¿ãX^èm½AGNbll3FGL J1327.9+2524NVSS J132758+252750?ïû¤.D?ë??ÑÏ©$£?AoFïP'??ÑÏ©$"?ïý}*­¼‰?Oÿ¤+Qä÷?4ª'¸¶?Oÿ¤+Qå?ïÓÏI3t?|² "û×þ?v[f7Æ1?|² "û×þ?ïü½¶)î)?2Ƽ"×(?:N°Ž­%?2Ƽ"Öé4FGL J1328.5-4727?¤4çrYéW@-ã
£3vÀ9tµÙk@ÁÀ;ÀŒŸ5@ áWÕ©ë ?ÿù6Òúä7?µc`øh\
?…³'Eæ?Üój:±VÐ@Σü¿è8ÅÖՏ?îAdÿ‰¯¿â]"Ð_¿áPj¡3–Û¿Û®ˆ^]ÙO¿ØVÇaþͦAGNbll3FGL J1328.5-47282MASS J13284063-4727496?ïñòÐJ?]…èš?]Â_kÒþ?]…è™ü?ïù$ÿ§6Ô?e—bT?Klc$°"?e—bP?ï¿eþ?€h!Ò"$"?€<fºÀµ?€h!Ò"$"?ﻯiÊÔ?t3Z=——?;%Jù?t3Z=—™4FGL J1328.6+1145?ËÕí4х@R¯_Ô{îÀ;q3JEžÀ<¶èÒ¼ÐÖ@"&6oÓ¢?÷÷'#'?ÔÖNád‰l?ÇðZpŽÞU?ôÏsÀÁü@©_àˆ¿Â¸G"£é)¿Õ¿¯'ä÷;?Àˆ]¥¢'¿Þ=—$Ê9Ê¿"uUËFò¿ØY9W9£AGNbll2E 1326.1+1200?ïóõ_z=?QíÝæ8d?XÅA†J?QíÝæ8d?ïüä\˜;â?Q[.¦ØF?8Ý> íZ?Q[.¦ØI?ïÁ)¿{/û?€ÝÖÎYÃ?k Bh?€ÝÖÎY½?ïèŸp/ïƒ?[(iÆv{@?g`Ð~'?[(iÆv{G4FGL J1329.0-5607?îh¬º‰G@y bvÞÀ7ÛjUß/¦À;ßTŽÍŽ@ÆCß}Ôl@Ì=s(? ;~.ˆB?½±•¹»"*@STâ°cà@º•¼?`é¿Æëðÿ\+¿áŽ›¤5Ôοå‰AAé¯\¿å¤º|h¿ëË7×âr¿åÀ~SÂöAGNbll3FGL J1328.9-5607PMN J1329-5608?ïÞp»Jâ}?t@ϲ%µ?pÇ¢ZŽÁ?t@ϲ%µ?ïʎ9XÓb?œ6Gï)?z¸ãS–NÁ?œ6Gï)
?î™kÃ'û?œ"\Íp†Š?¦iCΖÐM?œ"\Íp†‰?ïöÃ÷è,?E,|²Èß?Rx/§åo?E,|²Èó4FGL J1329.4-0530?íü·ØñJÌ@LçáüúÀ:¯'m-*À<P*º¾­O@§/¬@ti
à"S?ÉAV÷Þsh?Û£Ñ@yí­@ö¤^ïy ?ý¾£»º¿ï6¯õ%±j?ïæC_¿Û1W{fþ'¿ä'–NÜÝ¿ëFQˆˆÐ¿ïÿŒÝÉtSAGNbcu3FGL J1329.1-0536HE 1326-0516?ã~ÏAZ"?ÉD!˜©ñ?Ùa}K»×?ÉD!˜©ñ?á-טh°?ԋèHÕ¥È?ݤPÏù. ?ԋèHÕ¥È?⊖ãE#?·˜R'Ðj?ÚêÒ9tŹ?·˜R'Ðj?ѳ‡æþµ?µ(úÇå?ç@&<€¥?µ(úÇå4FGL J1330.2-7003¿©É¥§ÀÀ#éêÀ8±òAÑ[¨À;Ž¯­Uk@®b¬©@Ĥúö«Ã?¨VsÕå¡?ÂéËÎ|z@€èÈ«ÕÜ@ÁÝFl è?ÃÌàÃÏ£¿á§@¬m‡¿æ³˜H`¿棖b'$¿é,Ân¤ù¿ï÷`Ÿ'".AGNbcu3FGL J1330.1-7002PKS 1326-697?ïâêãš?hDì¦X?môüg?hDì¦W?ïù5ޔZa?b|oZy)ã?K(…®–}?b|oZy)ä?ïos—ð"?ócï5O?'Qû–?ócï5S?ïþÌ×CС?Q&°V+?#2‹Âö?Q&°V`4FGL J1330.2+7002?Ó›O@G\xB0üøÀ:S¯Ã§ŠÀ<µ"Î~}´@BÊáæ'?þ2‡V ö…?·ê"ßph?°Ý'ýuâ?ø^–ÞÔ6N@
ÂÚq{x¿çéƽ¿пÞ'</Ü¿à	¦ý…Qc¿ÚÔ¯DP¼Ü¿â{Ó {‹¿Ýx"á{°{AGNbll3FGL J1330.6+7002NVSS J133025+700141?ïÿ+ p©o?¿ë…oj?‹ñêÒ?¿ë…o`?ïýl¸™Jž?Kcr]Þ&?4š;5«V?Kcr]Þ&#?ïôÆe2VÈ?lf™ì‹µ°?Vs5›RqÊ?lf™ì‹µµ?ï÷
½®m›?<í%ÞR'&?Q䄣$˞?<í%ÞR'4FGL J1330.3+4441?á%˜Ý"é@Q²–»˜ÇãÀ:qy¶ViÀ<©-óXQÑ@`;€^µ?þ˜DЩ*?¶ÿ{?Áh§HÙ¸™?þTuˆBYA@u>Òx³E¿ÝG"Ô@_¿ØEL»D&¿Ü⛠ÚÖ{¿àF@V1dý¿âù|"MÀ¿ïþËê'QAGNbll3FGL J1330.0+44371RXS J133021.4+444117?ïڑt‰²2?pÓ‰'†©?r·E»&æÂ?pÓ‰'†ª?ïó_®C˜2?oûyÅ¡8?Y@£xϝ?oûyÅ¡6?5Åøè?†XˆÁŒ?ˆÒ2ŽÆ	?†XˆÁŒ?î권ô¨?†€îÕm?¡X—0µŽ?†€îÕl4FGL J1330.4+3157¿át[Ȓ@TêòRÀ;q–EQCÀ<°0Š‡@>u–8Ê@A&ÜÛ±?ÎÓʗé@K?Ò÷ ¥U@R]šåÉô@ÿTWÆ™?á拺³Å•¿»Ÿß?&l·¿éÓÛ·lé¿ßâWcJ¶¿ïÿa_3¿ÞP·þ^•7AGNbllMG2 J132953+3153?ì~AVD'ƒ?¹Ê·N[ƒz?¼
õMÛká?¹Ê·N[ƒz?ï/{žÈ?°î¢s6ìC?šЌ&ÿ·?°î¢s6ìC?ì8B|?§G3ŒðRÌ?¾;—5ï,?§G3ŒðRÌ?ël°ø?«+­¥¦Ù?ÂNõ<È?«+­¥¦Ú4FGL J1330.7+5200¿ãÊ¥´iª@P½çXÀ:*q?|ÌÀ<€ç"øoé@–A»6Lm@'"4H?·ª4??¡±…c°?çsqF"9@ùP¢"пæ	—Xv¹›¿å	Ý.Cà*¿åC‡sý'Þ¿ç•žvx,¿å'×="
9¿ïùía—ʍAGNbcu3FGL J1330.9+520187GB 132842.6+521750?ïý=áí«?.Ðãà‡‰?6ð'§ö÷?.Ðãà‡¿?ïüÝÌõ©n?R+Ú‹Ο?9˜R´–m?R+Ú‹Κ?ïëL;rX?gýÍB5j?d³Äê©(?gýÍB5c?ïÜt'LÌ?av¥ý?qÅõlYš%?av¥üú4FGL J1330.7+2933?êšzÒW‹@T@ò@úœÀ:'ßBñÀ<…0¹o¬@Êiïۛ@›Û ¥&–?ÆšÍ Y¼µ?ÑÃZб@œT\È@H‡RŽm?ìs€àæ	_¿Õ]ê–â/5¿åÑu=™¾ƒ¿ìTR½'M¿íÞæÀ=ó+?åYã¡$¨VAGNbcuFIRST J133101.8+293216?ï§<½Ë¢Ÿ?…©¯~(?†0ЍX\?…©¯~(?ïû_j"?WÛÄE},	?CŠ'Uï­)?WÛÄE},?í
׬^V?£ð{X^Q?·¯¹B
T?£ð{X^R?ïÜÀ)#T*?cµ8^¿çÄ?qŸënUë\?cµ8^¿çÁ4FGL J1331.0+5653?æ\h2«n¶@M´k&¿‡jÀ;Zw'ÔáÀ<ïcáPèP@ ùŸõÿ 1?öûUvT?ØB·ÀK41?ÒFŠþÌ#?õb¥ç…¶?øj¶ü¿â°›ÿ$Ô¿ê[a .Q¿çp5½Q.Ç?ªÁdÂUD¿ßZ_U¿ÚƒT]ÐAGNbll3FGL J1330.4+5641RX J1331.0+5655?ïù²G®Â?D5•@z?I7ªáDû-?D5•@"?ïó¯luÔ?zzbáÏNV?X¡'æZ$?zzbáÏNU?ïŸé‹fyI?†]•èÂ?ˆ&a­Â?†]•è½?ï£ùã[í?vˆµCÀÜã?‡º‡)ä?vˆµCÀÜâ4FGL J1331.2-1325¿î½š8¤O@H'M3H,À9™X¸'úÀ;ŽŒ3‰M@4@#‡@èŠÛ´ï?Ã>êáà°/?Í&ö9ÔA@ PxË@4j­óò¿ç¬h=Öû$?À‰ßgY+¿æ ¤_ñ,S¿ë`ö í¦¿ã°W¡&«»¿ïÿþøþ"AGNbll3FGL J1331.1-1328PMN J1331-1326?ï—@%¶º?'
;Àœß?Š/ö'|Q—?'
;Àœß?ï÷¦õšÏ??cŒ(C˜?P²Êa€ˆ?cŒ(Cœ?ë.¢y¯{?®';¦¥¨?ÃGµvB?®';¦¥ª?ïJi¸ƒý?Y6…L±Ì?ž–²Èï€p?Y6…L±Ë4FGL J1331.6+1711¿èõ½Bo)@SEbàŸèÀ:@óÖ&À<ptšÐ$@-…àT>@Á]}‰˜›?¹<ÀO»Õ?Æí|Õ¡?Âi;,ü¸@R:«økâ¿Ý«$[¾¿æ1L©%þ—¿áëâ—°¿åTÍ·®X¿åÚ;€ÎÜ¿Òg'áC§JAGNbll3FGL J1331.5+1711TXS 1329+174?ïæŠfT?f|¦¦?iu癫p×?f|¦¦'?ïüAølº?T'Þ¼m?=ð<Ÿ,"?T'Þ¼m?﷞s"?ƒÓðü€@ß?'~ã8wi?ƒÓðü€@Û?ïÝBò_*"?`0êՀ\e?q^†Ðj·	?`0êՀ\f4FGL J1331.7-0343?¢?ULdܝ@LÓ;÷'À:]òœj.rÀ<Õ¤ãc@¾k[m¹í?ùæ(S`'?ì1d™ˆ?æB^
ÒQ?þÛÐ@Ô@T@¹Ù€?åðg¦ØF~¿çQHÇïî:¿ã&ØaU…n¿ïÿèã«6¿¸š¬È®¿î:
BâMAGNfsrqPKS 1328-034?ïó}ká¿?m>>Ž /±?Y(<ù(?m>>Ž /µ?ïüñýhù?S›H˜×À?8p̸BÄ?S›H˜×Ã?ì:Xd:‰F?¨xDJ¥Û?¾-<Þ+µÖ?¨xDJ¥Û?ïíº¯<xæ?`Aí	ƒ?bEPÇŽ?`Aí	~4FGL J1331.7-0647?ïÿûäU€†@KY†üÞãPÀ;ÂHåL À<žw{@áqF>RÌ?ü™ƒyœ¤?Ïm"ÝzÅ?ÓW,u©Ð@»
,©¬@6ŒØ–¸¿Ë»±\"?ïø €´ã¿ËÊ+éÔ¿à›¾'1H"¿æW9''¦¹¿á¹
"BËAGNbcuNVSS J133146-064632?ïéfo¬Ô1?nˆæ_­?f™S+Ð]?nˆæ_­?ï³ó}/?•kc‡'†Î?ƒ:`´8Þ?•kc‡'†Ð?î®dTy¥o?—KñäÅ?¥º¸e©?—KñäÃ?ë/´¨¹¬?§²Ñ
b¶?ÃçA-]P?§²Ñ
b¶4FGL J1332.0-0509?ãJhH—#N@Läy'¼VÀ8¯ ÄÀ;'ŒÂÂ#@	"'›Ø@&Ð& û? Áø»ñÚ?Å[ôœî¹@ †/Y‰ß@»û¢£-—¿ÓéŒÁDŽ¿á•"Ì'úò¿ç–ªÁµ£¿êqü!#;C¿èÜ"¤?¿ïÿ±Æ·	AGNfsrq3FGL J1332.0-0508PKS 1329-049?ï°Ù:´¶¹?'îÒQw>¸?ƒÉ±RÒR?'îÒQw>¹?ïãG»kNr?€½øç#?l¸D"±Œ?€½øç#?î(gëj?›{Ô-_ò?§-yO¹€?›{Ô-_ò?ïøʊ˜®S?AϚÈR
?LÕ՝F¶f?AϚÈR4FGL J1332.2+4722¿í•Ò¢±$í@Q篷éÀ:]N[­¥ÀÀ<tZ5Ö{¢@E–hâ˜@Å1Àll:?À±µY¾D?²†¯‡µ#?ïOo^²'å@
$¤¥p;?ï¿àÀŸ—à¿ãiWaæ¤å¿é-h]â^Y¿æ°<g™í¿ëñ§½s¾i¿ïí…èÜÎAGNfsrq3FGL J1331.8+4718B3 1330+476?ïú³µ
¾3?CÙPÄâ?E1+É36?CÙPÄáô?ïüO£šðÑ?U¾ˆK£?='ã(y}?U¾ˆK³?ïåÊK"Òš?iĈ'þ{Ê?j5´l-et?iĈ'þ{Î?ïä¿ø7J¸?[™þ1?! ?k@ȵFÆ?[™þ1?!4FGL J1332.6-1256¿ãnjޖ€@HYµà÷üüÀ8ݜþ¨èÀ;.
—~6@†/8§¼G@8"üS£? øÙßɘ?ÀÄEª.<S@ØFèòA@õxèt¿ÕH­ûŸH¿â׌™¿æ=é¿æЖP8ýx¿éL!`ø¾B¿ì
Gahz¾AGNfsrq3FGL J1332.6-1256PMN J1332-1256?ï‡äÏ'g?‹§:2bOn?Ž:Ì6&x?‹§:2bOo?ïæsà?}÷'Zäu?i€Œèðá?}÷'Zäv?îçê3°ýn?—…×ÏÜ3?¡\Äð)-?—…×ÏÜ4?ïŸuZf?{ú­üŽp?ˆ"©y¿f©?{ú­üŽp4FGL J1333.0-6626?æl.ŠÀ&êÀ9æRlÀ9åüágŽ…À;|Ëëü<ý@<r‰à>@9Eßaô?Б} <5?Òb÷{Ìÿø@3.`e›e@QøV¾R·¿· o Ê$ý?ëñ_ˆ{º¿çGQÞD‰¿è³¾smµæ¿ïÿ틉5ž¿ä9óEAGNbcuAT20G J133254-662826?î³Z¶@à?´%/Õì¶H?¯äÊT›ò?´%/Õì¶H?ìriU™°^?Æ;s¯q?¼lµS2}?Æ;s¯q?çsJзa?³O:oHc?Ñj^'=è?³O:oHc'?êÀ£´cá?­/Ózl¸?Äýq/Þp€?­/Ózl¸4FGL J1333.2+2725?ëÏضg@T,¯¢ðZqÀ9åkÅKÀ<ƒˆ×@yÄqßk`@/${	‹š?³5ëId¢í?­/)ä*—?öôLfàà@
"ÞCÿ ÐU ùè¿ãX˜GŠM¿äH3
‡¶¿äbYDzä¿ç#…uö&b¿æz˜í¢/jAGNfsrq3FGL J1332.8+2723MG2 J133305+2725?ïùÇÍԕ??Tág\?HàÈ­¬??TágU?ïûXí?^N?W=Ì£KÝÍ?BœK†Éj?W=Ì£KÝÊ?ïí`8üç?f…ä£Áõ?bŸÇä$?f…ä£Áõ?ïåap^ûð?U'ßVä±å?jž¡?U'ßVä±õ4FGL J1333.7+5056?֯Ñ@P7Ù+à‹À9QpXW¯êÀ<&€Aÿ@Ž5deÛ&@oZµ?©Šނ›•?¶ðBrÁ=¢@äLæb @QúÝv?ßÝE€gÄ_¿âïÕ¿ä•`ß鵿äl¥¡·¿éJS
iŽ¿ïüÒf(SAGNfsrq3FGL J1333.7+5057CLASS J1333+5057?ïû\/ˆyi?8RZy?BAÞYÑ?8RZV?ïúñó¾?_±jÄ ?Gø;Œ1Ý?_±jÄ ?ï'GOK"?†‹?ÏëÖR?‹n?ì-?†‹?ÏëÖV?ïþBîÜ¥?‡ÿ'ñ±ï?+Ñ5®¢|?‡ÿ'ñ²74FGL J1334.1-3521?¸Ú±p2@:´óý">6À;†qž¨ÍÀ<µ—îáË@",Ò£üI?û e›eK´?ÇÜìš"ì?{øVñÜÚ??¸=¾./?üKÛÙ=§¿îGø½Ÿ¤?¬ÜUÖÌ?ïçB.x¹O¿º‰#ªª
/¿ê<Œ¾÷Y?Ï1úcˆænAGNbcuPKS 1331-350?ïöÁò¾Ìå?K
ØÒ{‰%?R|'f1·?K
ØÒ{‰"?ïü•0yV^?]\¦¤È¹?;V|5M}?]\¦¤Èµ?ïy9—oŒ?‹Bžàf±?ØÝ-"?‹Bžàf±?ïÒ뉟KK?lxñ"±'?vŠ;0ZZL?lxñ"±'4FGL J1334.5+5634¿ÔŸ/Ãi¾@MÈà"'À;J&˜=™À<¾2‰}Ã@ÅSÅ$ù@÷çbzH›?ÃJÕ¦»?¿ b3Ѿ¤?ܦÆ0<‰@£úü5>¿î3(¶ØnÁ?ï®þ`¿¿çêUp
¿ã½¢W®<¿¿êøýâïN?Üá­å+}AGNfsrqTXS 1332+567?ï'øäöƒ?ˆ}þApûS?‹ÆÂ_<q?ˆ}þApûU?ïúI¢¿ö?bÔ7¼"?FÙuÀ.j?bÔ7¼""?ï
u·	a?•43¿{g?žQIܳ×?•43¿{i?ïÒpÌBäD?hœ›Çým?vǙލޱ?hœ›Çýn4FGL J1335.3-2949?ïý9Ppð@@
=¢ø½ìÀ:_ס<%JÀ<i'Où<—@ÏÄùÛ?ÿ@Íù¦J?º[ˆ'ßf?›'ù†-?átþªëQ@é
<€?î&üX«'À?ÓsºÂ‰'¿âþiȶe¿Òi7;«|Æ¿ån)¾ÀD©¿æ¾[ÏßAGNbll3FGL J1335.4-29491ES 1332-295?ïýc£Þ°?4qÄKsi?4çŠá
v?4qÄKsR?ïü€"»?SX'6֓?;ÿ›Ú' ?SX'6֓?ïí­,‰B?p½È5"º?bRÓ÷v½'?p½È5"®?ïÎ-høø?f[úi?xéKóƒƒÇ?f[úi4FGL J1336.2+2320¿ä܇ã
L?@SÌs-õÑÀ;:ØC""À<ºoª²Æ'@½mç94ª?û.ʸöV3?ÓÖBAn	s?ͽ—»!ú?÷إ̭Ã@ۅ9D†?ë·Ç'
0Û¿ì=¥b$¸F¿ÍºÞæ¿Ç°j–vÏj¿ç€…@dž¿ïÿÀªšëAGNbll2MASS J13361219+2319581?ïþ2e·á?'Í멤cs?,Þ¤ãª?'Í멤cì?ïûµx¶NÀ?T™Å"õ_?A*&Äø¨?T™Å"õT?ïÍ"†?zݎZ‹n÷?ynñÿ¼·Æ?zݎZ‹nî?ï×ËC¹Fº?`‡	{ª?t^#\£º?`‡	{¬4FGL J1336.2+2053¿æ"¼Ýòºù@SÿëJÀ:ã
æãÏHÀ<•¬Þð¼@¢3k½=c?þԓj«p?ÍÙ_m=p?´".›säS?ê–
ΐl@,.Œ…_?ﺌޠ3è¿äÜÃàj
¿á‡—¾V迼e®Ûu1/¿áƒ"Ê/c›¿ç×_f˜AGNbcuNVSS J133612+205102?ïÿTB-±7?¸&eÃ?wºIØý??¸&eÂ<?ïýyæÆ¡ç?Iì{¤¯Ò?40ÉÊðÈ_?Iì{¤¯¿?ïø£~ó?\F'|jC?MsÎ3Ë?\F'|jJ?ïéèk¯è‹?TPã€Üõ?f"Ps?TPã€Ü4FGL J1337.4+5502¿êo<eø@Nm©CZÈ£À:ôå‹àssÀ<¤ÝŸ'ç¦@_o̵@Æ"ï¾?ÃãŽe?•g³™ú"?Ñrd`ý›Í@
Íî¿›\¡õ*0¿æp@o[Øn¿î8¯6Y¿ÍÈ#à{Ö¿àAœbKό¿ïí…>˜ÂAGNfsrqS4 1335+55?ïþ´»ï–y?$¹ü`êw.?$´A˜d/?$¹ü`êw)?ïý=шØt?P²©Ð'u?6s¹<^4?P²©Ð'u?ïã'?pÍ£U§?lånçôç¿?pÍ£U¥?ïþ›ã‹~?%p0j¶Lß?.vAÇH0m?%p0j¶Lä4FGL J1337.5-7802¿éQÉ5k¨ÆÀ.ÉÄüó0À:¾eò£ +À<jGW­eÿ@l/µÐ1@¬¸?wT?ÈÍvÀіá?¸]/ÛåÄ?ñtVéò?é&ƒZ?î48Ùeb¿éÄ×5›J¿å"åÕ²O¿ÐÓDá"é¿æŽBM'j¿ïÿ«Ÿ7=AGNbcuRX J1338.2-7801?ï÷˜ðh–8?†78–æUÒ?PÎ.ӌÇ?†78–æUÒ?í«Ba]^?»ÿ&Vu?²¥ì÷ý?»ÿ&Vu?ïпEKå^?~Vp¬*H?w ]Z
Q+?~Vp¬*H?æÎt €?²ÁÇåŒ?Òcãö¾ÿ?²ÁÇåŒ4FGL J1337.6-1257?íj'êkcç@H0W\gÓÀ8¼^ÑF¯À; *o?Rü@€|»@p…ÔÀ·?ªâ¹âÔú?Á·œäÒ¨@÷x‰|ì@;ñ®ƒ‹?ì赖Ob>¿ßI¼±K½¿åºß.Ï d¿æÉë	ζ¿çüQ¿æ4}¿ëãú !°AGNfsrq3FGL J1337.6-1257PKS 1335-127?ïèhî©ká?gGÑÉqÀ¼?g—V"·?gGÑÉqÀ»?ïãfÒî$?€øÜ[6ìì?l™-ûÜE?€øÜ[6ìì?ï›yœTÍÎ?‡~n¦0?‰!˜ê̌3?‡~n¦.?îÐKûI9a?ˆ/݁ÛÛ?¢û@Kliô?ˆ/݁ÛÛ4FGL J1337.9-1956¿î}¿®"
4@DÌsWæpãÀ:ó/p0ÄÀ<;+äŠX´@Œ·ÔCé@¶5¾þ­ð?̇À键£?¢(^Etm?ÕØÙJ‰'@
lš­•Ïà?튌Jü}•¿é¨USïk]¿çN'ÿú ÿÝEâb`Gh¿åšVÞ3&ž¿ðAGNbcuPMN J1337-1958?ïÿ+±kĚ?'tÛS?‰Ò‡lðo?'tÚ§?ïýº' ®,?P
H=Ÿí?2.ÆúŽ•‡?P
H=Ÿí?ïâaÀÖ¹Ì?s捚;'?mž?)F2â?s捚;z?ïú×¥we?4¹@RÎÓë?D£éj"l_?4¹@RÎÓñ4FGL J1338.0+6534¿ã"…cûØ@In¤"‰—ÄÀ:d¸ÄL0À<…Ö9ïæ@´`àÀu@!‹…ÚŸô?ã%Éé±?¿6Ü
,~¹?øôèû¼¾@
)Öð? °XÍÌ|¿æY	áÖZ¿æºl­¨DW¿ê"öÕ®¿ïÿµÝœþ©¿ïÿ‹Á>ÏAGNfsrq3FGL J1338.9+653287GB 133543.8+654752?ïý]ž"
_?4bãW²ŸÍ?5ï"ÿo?4bãW²Ÿý?ïöÕWŸ?i!ls÷!?SÐUçPÀþ?i!ls÷&?ïäG—â'?lúÌq'w?k¸hmêB?lúÌq'l?ï'ÞK@6?tû«´z.Å?‹ˆm9¯òR?tû«´z.Ã4FGL J1338.9+1153¿àô#PXƒê@QÈ\|ؙÀ:»WYƒ)À<XEq
‰@òv`¯m@@uá;ÚÂ?³AwïzÌ¥¿–gڄÆMØ?䆼²£UÛ@ûû!ÉÔJ¿æÁáìï'¿Òƒ`½Z¿æy¶Vi¿Ýá‹5RÈ$¿Î†Ï'y꨿è'?
äAGNbll3FGL J1339.0+1153SDSS J133859.05+115316.7?ïü¶¯mŸ?3¢m¾Åƒf?:J"—£®?3¢m¾Åƒ*?ïü³Á
'æ?U46œKéô?:a÷–ÀØi?U46œKéð?ïõ?å0Xž?a÷žƒ'½ô?U€5ŸNą?a÷žƒ'½ú?ïýøÍÕ="?$;ñÍ%#R?09'Vàv?$;ñÍ%#H4FGL J1339.0-2400¿ê–ÀŠ@BËw[0À9përáÀ</;©#z@ÐÃ7LÈ[@÷3¨£ù?°k̬Ái—?®ý&¾%.?ýt,!Æú%@tn}·÷?äuÞÿT^¿âJiæM§S¿ãqø -à¿ãô±œ]™¿è~¶ôô3C¿çR¾éµ;AGNbcu3FGL J1338.6-2403PKS 1336-237?ïó}i"?Sä
€¦¯?Y-ãÖ×ß?Sä
€¦½?ïü'Öêîh?TbÖ0Z?>ÁH¨Œ·Š?TbÖ0h?ï×+X&"k?r{úáÄ%?tjSìµÊ'?r{úáÄ&?ïñ4Â'+?Hò‰nàk?]–{±©È?Hò‰nàf4FGL J1339.1-2620¿Õ'ƵáA@A¨hۋ¬qÀ:u\€3—À<o'OÐ!ì@_y';|-@RÑ84$?€*ä ©?¹LuN‹©A?öÈÝ•.@
'áG®{?ïJùùUÁÓ¿å½K_¤Ö9¿ápXô©¿âÙs8ÜÀ`¿äÅ"}c¿æŠD'HAGNfsrqPKS 1336-260?ïüìiˆ±?28ƒ˜i?8œ³ºww'?28ƒ˜?ïý×rŒz²?H¦Ë&.O…?1Dkœ*i]?H¦Ë&.Ok?ïòcºˆÞl?i´áÓéÔ?[8ŠîC&ö?i´áÓé»?ï÷‡%ö3v?8Pú6…ÁO?Pñ´™j?8Pú6…Á"4FGL J1339.9-0138?ïF\N¥Ãí@Mzj~ùÛ#À;=[XkÀ<ÜãèrDÁ@‹‹ØeÝ@ñ·D¥?їÆÆ"Ž ?åÀGƒLP;@Qͽ"©@ ß=è˜Û?ïõêgèF¦?ÜWžbP2¿âG~>œ¿å @LÜ'¿ïÿ¶>@£?ë\e[¤k…AGNfsrq3FGL J1339.8-0133PKS 1337-013?îËÝ5²?ª¡Îû¬T¢?£B/?¤á?ª¡Îû¬T£?înˆ=ùTE?Á/º¨Õ§Ä?©| j»¸?Á/º¨Õ§Ä?àÛr&š'œ?¶½arI.?ÞI²Ë°È?¶½arI.?ìrdõ³™Õ?ª>îÜþ?¼lØRc1\?ª>îÜþ4FGL J1340.0-1501?íaA¯Iû@G›¥ãSøÀ;XB 6mÀ<®Ö0ù@!j¼<ܪ:?Ûeºnü7?àcÞÌ©'^?îȐB@™½ÆŸŒ"@qëô…M‡¿îôŽŠïˆ?ïñ4?ø"z¿êì>ý–Ä'?²Ë;A
€5¿Ñ΂#Ü(4¿èMnGÜ7¤AGNbcuNVSS J134005-150314?ï¡n¯Ød?‡Ÿ‡h	#?‡¤T	æúE?‡Ÿ‡h	#?ïö™ìì?l1Ô¹½ÄU?RÌ&'à÷?l1Ô¹½ÄU?ïY§Ibí?áÀ¦¯…?"ËÓ¼Bs?áÀ¦¯ƒ?ïÖ8ß#פ?qÓA2Ç?tãn-W?qÓA2É4FGL J1340.1+3857¿ëûîYM{@R™çW"À;3
s†
À<°¦°ÙQ@@§;N
@>Ü~ñw§?ÌӒy>Û2?Áîj@æz?îuà÷üü@@躹¤Ò?ïÿȂeJˆ¿ä­v€d¿ë]Ä×5¿à °)¿é•ã+³ã¿ïßÓo~=AGNbcuNVSS J133849+385111?ïýÞ#ô*Ö?<&ζ¸,?1à^©KÌ?<&ζ¸V?ïùG!Á1?m§ËœÜ(?Jãxûÿ?U?m§ËœÜ/?jâ¬?ˆë™z³~ü?åGyÔj?ˆë™z³~ó?ïÙ3¤í&1?gâöÊnö?sf-‰lçE?gâöÊnó4FGL J1340.4+6926¿íRÌÀñÇ@GŠpCßÀ;µ?ÇÀ<DZ«ß{@dlƒ¶ÙF@v†a®pÁ?̎	Ãx:N?ÂþgN˜¿?òMº°k@À"CÆÿ-?ïÚKäÚá¿jÓaL²Fu¿ë:ñ£EêÆ¿ÙÛˆü¿ïÿÿÊPË?ï½%?T©¦AGNbcuTXS 1339+696?ïþ¾Dq2r?-Ê6«sg?$¸ìØêè?-Ê6«sg`?ïýTµ!?P÷ûr'‰[?7}ZV÷|?P÷ûr'‰]?ïiăà?a|i¼µ­?'Ý'oƒÿŽ?a|i¼µ«?ïÿµöJÒê>û¦‰ü숿?'mKE=u>û¦‰üì‡>4FGL J1340.5+4409¿Æ¤vðä@Q"¦ YŸÀ;•/§xÀ<©u¹À€Ž@"!ä*7?ù¶È™aev?Åʨ…DÎ?¬°Ä¿žLB?åš>o§WÈ@ùŸM㍮¿èìðùÒ¿U¿ï"8Á½z?Ü5-vÇ¿ÏöÈlàÿ¿Ø:ÀðÒ¿£-oàô³,AGNbll3FGL J1340.6+4412RX J1340.4+4410?ïÿb»(´?ßsO½«3?¨šé|L
?ßsO½ªJ?ïýó<NÞ5?HÃò	g3?0f‰U·?HÃò	g?ïú<<?C<¢f'¹?E¿ƒ÷
n?C<¢f'Ï?ï÷óÆÓÜ?@蝈ÿÕ?PsÌXH
?@蝈ÿö4FGL J1340.8-0409?àO5òöƒ@LA]€ä–îÀ:Tò÷ÙÀÑÀ<^=ç™@µ|I| º?þ®³Ý¾?ÂÓë9Ÿ]ÿ?˯D%ɾ%@
jOv@'g…d¿ïԖZIør?ïÿþBe«+¿Ùì ºŠªé¿áÒ°;œŽA¿å®úS¿ïúX¡+ß,AGNbll3FGL J1340.6-0408NVSS J134042-041006?ï¨/ú±E:?ƒmkô?…ôS®±Ó?ƒmkô?ïÀ²Sxw…?šã"'oIâ?¦ÖCÄ=a?šã"'oIâ?ípŸ:˜u?¥pvú8Õ?´{+?O?¥pvú8Õ?ìš4Î
ý?¢ípŒÈm?».Y¨v?¢ípŒÈm4FGL J1341.1+7433?ä†??)ÿ@EI¾ó(À;õÙ7>Z¯À=8XÍ@!m¡™?ý>½c£>?ξ¿ƒc!b?±í{˜ý'g?èÙ᝿C!@Wê°¢¦¿ð?ïÿùJYQ¿ß ªº©3À¿ÝmS?˜j¿é"Î^G^
?à…ª.<SmAGNbcuWN B1340.4+7450?ïþ¹kèY?'n›4z³±?$n9AzŠä?'n›4z³·?ïþpµ9—?CQâ´1ÅM?.Xô¬f1?CQâ´1ÅG?ïœwûř?‰¢÷Ò'?ˆâ™¹K?‰¢÷Ò*?ïô›H¨®.?K'€³O…?VÉn®£¥ ?K'€³Op4FGL J1341.2+3958?èח«É@RaÞ¨—cÀ:´4'D¤À<ÐÚx†ú@ ›Ó¾®{ÿ?þUÃKCË1?¿£«@`¿";$wj¬?Ö¢WBÜôb@üP#ÙÎé?ïúÖ*C i¿à*·ß)ñ–¿è?¯Èe_¿¹¸þæ$¿×ú3ÂûڿގH,¿{«AGNbll3FGL J1341.0+3955SDSS J134105.10+395945.4?ïü;ßjêß?9"mתٽ?>!¨©
Ø?9"mת٥?ïûgÎ
Ä?VÎa&×1?B`Çˬõ‰?VÎa&×.?ïñ؆ã»?aH=2¡ËÔ?\NóÜ8‰@?aH=2¡ËÊ?ïÚ{<9Ì?^"†åO­?rÂaãtT?^"†åO£4FGL J1341.6+5515¿‡ž·JlŸö@N7°ËæÀ;«GhGÀ=Í 1cO@˟P<ÙO?ÿ0–‰B?Õ6]ŠÒ?ÄAꛔÆv?ðÖN™@°	j¿ïÿ3Qf$!?ïþ5$¤ú÷¿ÉŸF—> ¿ÝFéÞÖd¦¿ì.U'ÙŒ?¸Y:®Ò'AGNbll3FGL J1341.5+5517SBS 1339+554?ïæÄR+n?e'xUãû×?i;­åԑï?e'xUãûÙ?ïújÎâ0v?cneaŠ?FTÄw>(O?cneaƒ?îÿ='ðè?"bl˜õä? &àñ~È?"bl˜õæ?ï¯5$(R(?rË "
Ùk?"2¶õëuÅ?rË "
Ùk4FGL J1341.7-3907?èìr$#ÝN@6·Žâ†ruÀ;›¡Ÿ!˜×À<Á_s-F@!ë¹½ûN?øŸåÉä?ÖFlÊS?Ĝ:HPPÐ?ên±XÒÿí@AP5ÍlZ?ïâkªÛ
¿äòõÒ-_¿ïôo"͊?ï­œ®÷пë‡ùÞþ¨'?ß¾F!L€âAGNbcuPMN J1341-3906?ïùV†• )?My]_ì=§?J¥å©[é?My]_ì=•?ïüŽônþ?SóÊ)¨?;ˆ_ˆ}?SóÊ)¨?ïR9ˆ¥»™?8Ž^CqQ?•¸ÎëHŒË?8Ž^CqP?ï÷¾%j ³?Q,ó´õw?Pƒµ+¾™ç?Q,ó´õs4FGL J1341.8-2053¿Ùæ˜Ä.o@D:[–(ËÑÀ9ÊàÆ~ÔòÀ<†Ñ?ù@ÿ¶YÃÀµ@t"« «?¼~)¦—ƒë?½[K?Äf!?ú4§Ý);c@®ã‡¤z¿ÝF—"Ûâ¿äñiϧr ¿èÂSAp²¿êªüóF¿éØêýºU|¿ðAGNfsrq3FGL J1341.9-2053PKS B1339-206?ïÿ®'»?›©ôÙ=t?Ê?[–?›©ôÙ=Z?ïý5ÁÏñÞ?Q[*¸EL?6Qñ€qÜ?Q[*¸EM?ヒýÕå‡?}¼8U‡Ý?€]Š†žr?}¼8U‡Ý?ïüëÑ1¥?)ÞÿöV?8¡vrӊª?)Þÿö¬4FGL J1342.6+0944?äé'o݌@Q4Z_Çæ´À:||ûÀ<€"ï5­a@¬ƒV6C@‹°'ݾ?Â77º+Šr?¶ÎùwМ?õL{ÃŽ@ª²W*´4?î°ßóE2¿Ó֑ýCD¿àéâoܿߥk*±¿ç2F8Éu)¿æ–øÕiSAGNfsrq3FGL J1342.7+0945NVSS J134240+094752?ïøìbj4?L|8×Ä'?LNwÒW/å?L|8×Ä:?ïû
Y÷´K?\ßӀS¦í?C֘!.֛?\ßӀS¦â?ïçTìüV?sö,T	ª²?h«©ãÃ?sö,T	ª¯?ï˜wEà*Ä?qé´79ý?‰â.‡õO?qé´79ý4FGL J1342.7+0505?ÖÂ-I@=@P3 ٔ[lÀ:…̹–nÀ<z
Á$"@´¥§nïL@lFD‡ïM?¼èÁÊæÌ¿`àéè?rï‹y×m¡?ÿÓhõâŲ¿Â´†…ß¿ßíÞҞ¿çpLÎå«Á¿ãAãÀe»¿ëp8à?á¶?Á8AGNbll4C +05.57?ï[ð^q?'¬¬Ç«(?žüôô1Ì?'¬¬Ç«(?ïö'k±"|?pª¥±>)Á?S±(»?pª¥±>)À?ï'ò×?'Ù%ÍÿÁ†?›á¥½H?'Ù%ÍÿÁ‰?ï­!øsõº?tµ´CjÅ?"·ã'¨?tµ´CjÈ4FGL J1343.6+5755¿ïò³&Ì@LïQ½aõ¾À;CP8&·ûÀ<ÃÕ×7‰Ú@½ÃIâ¢@ÊOv`?Æï8&&Z¿"-"®jƒy?½*¸TÌ`@ëÓSú~?ïÞ>y¸R¿ë³â…›µÔ¿ä™V³jû÷¿é©YàÆÿ®¿â7EçjÞ¿ïú°€²AGNfsrq3FGL J1343.6+57536C B134209.5+581020?ïÿžAà­ý?
v]¨"?o‡Ô€c?
v]¨…?ïürÁ–õ?bk
9c¤?<ióHWt'?bk
9c£?ïäF.v?kÛæô2ÿØ?kýñ¹Ñ‰?kÛæô2ÿÑ?ïøBŽö?A›I60nç?MÊõǜ'#?A›I60nå4FGL J1344.0+6605?Ž©EmoX+@I™" äÀ:›wTË3pÀ<«"¶
+@–6ükuð@äìé¢Æi?¿8Ȑ‰¦?°£€ùÊ?íºÞEÆ@|™ÒÏp@¿á¹€¦ƒ¿â³Eqú_¿ççb\«¿æ¢ ©XS~¿â¦t©H›¿ãŸsbÎ+rAGNfsrqGC 1342+663?ïü˜ƒBOÇ?0ŠDTÿò?;;åíÄ?0ŠDTÿñ?ïý}à<?OQ-g‹Ý
?7Wäþ;?OQ-g‹Ý?ïïñ—ý7¨?a™þJvjg?`hÈX(?a™þJvj`?ïï"Í
%?LÅP"Ó?`k2õÚÿp?LÅP"ó4FGL J1344.1-7700¿Õgi"|À,è鳍aÀ:j{Ö:3ØÀ<_ÐJ/Ï@dá59°@ðÏü,5é?ÇߋÁ>Ï?Æ˦‡ÙL?ùÂ=ý'·?õÂ/)ä*¿ïïwÀOç?ïþõU9¿æRÝ^ˆ¿í©·ôÎs–¿k*ýžj¨"¿èk¦âWxAGNbcuPMN J1343-7658?îz¹K;{?±£k­ˆˆ×?¨TkLOH6?±£k­ˆˆ×?î•B—DÐ?·-UË]¥?¦¯û֋³
?·-UË]¥?êG]0"9?¶n4êFÉ{?Æâ‹?§w?¶n4êFÉ{?ë†ÊüGœ?³j)ü…'×?ÁäÔ†á?³j)ü…'Ø4FGL J1344.2-1723?ïýÞљ}@EÕ¡"úÖËÀ8ðÍ¬üÀ;Õàl¼Á½@.÷"ûR@ÙªæÈ÷U?ª´vØz?¿-¯e³¹@ORáNd@ãؖÚw…?Û´;ÿµ'¿Ùs8œS³0¿ã'Í¥&Á¿áš¤'D`'¿æÄì=ÖOX¿ðAGNfsrq3FGL J1344.2-1724PMN J1344-1723?ïýD[ƒ.|?8q_cÝ?5Ý#æŒØ?8q_cë?ïö¤'Ó:²?kÙ`…p£?R¶úYŠŸ5?kÙ`…p¤?,Á"?Œi^žK'?Œß4Ï»[•?Œi^žK'?ïý¯Ó±?#·­œ»?2gbwŠM?#·­œ(4FGL J1344.4-3656?í-ž/<¯@8¼%á;ÛÀ:6,PÀâ´À<G‹³ýÉ@Y/'éA@£Cœ7Ì?¸Ñæg'¬l¿tª÷ºâ?ã_v¼Ï)@:î¿»Â8¿ÚËÅ:Ý ­¿äpŸ¥LU¿ä´àFý¿å=µ¢ä›ö¿âŸÐJ/Îû¿Ô‰þ¼3!•AGNbcu3FGL J1344.5-3655PKS 1341-366?ïÎ	œ%"6?pëf²ÕÄ?xû1í=åq?pëf²ÕÆ?ïú«ÀJ?^ɜçY£?G§©PþØ ?^ɜçY­?ï¤?"ó%?ƒ|OE~p›?†ðÃ6¢?ƒ|OE~p—?ï¯gâõYs?p/‰þíå,?"&B©£,?p/‰þíå,4FGL J1345.5+4453?åQ ±»×@QM#c²WÀ7&Š
4›éÀ;q%SvŸš@|Bµ²)@^á77¥?‹›ó]|ªB?³øf>ßu@&y•în@ »ˆb¾¿À
lÐó.¿à Êƒ+¿ä²+@ "¿äk¾§›¿èÚ^Poˆ¿ìܞÁ̓—AGNfsrq3FGL J1345.6+4453B3 1343+451?ïÙlEÖ@?nÊJsœìÑ?sIð]ßí?nÊJsœìÉ?ïÑþyav?¾Ze¤?wÃyÏEˆ?¾Ze£?ï¹ê<|Â?ìàé"Û?…pàüOƒ?ìàé"Õ?ïèF‰"¶?`Õ?¶
ÊÍ?g¹vélJ?`Õ?¶
ÊÍ4FGL J1345.6-3356?ÀºXNˆm@;—BöÖÀ9ýžóu®À<PS@ôÄ@¾wÎm¶½@W]K4²?µž—°5gk?"?\6a»Ý?Ѷ»"i@+(wÃ[?ï÷À@win¿ääž_Ñ÷¯¿àýXsHͿ㣮¡£S¿Õú7¿	Ò¿áž$˜¼AGNbll3FGL J1345.9-3357NVSS J134543-335643?ïýÓR\+L?0ý¥²ª'?1em¥¢c?0ý¥²ª*?ïþÛ&¤¬x?;´	Ê܎j?"M•µ8ŠÙ?;´	Ê܎³?ïíþùÅÙ?mé•0è5?bî:'X?mé•0èI?ïÿ†eåùu>ÿÕ©Wë}?f†¢'Å>ÿÕ©Wë4FGL J1345.8+0706?ßS–Ç;›@P‹6¤û©À9lì®êc·À<7T+Ñ?"@‰gWË@P†å?¯6lx¤,?ªíŽ
t]?÷@ô@g)™¬c÷¿ÐB~ª¿ãWZYé¿åÎU-XþŸ¿çí`Á
ø¿è¯>;¤ò¿áìÈ×'šAGNfsrq3FGL J1345.8+0704TXS 1343+073?ïü¹Ý•ï?0×N°n©ô?:1S›;?0×N°n©ó?ïüœE`*3?O®ÝÌ©ð²?;Ôþ®hG?O®ÝÌ©ðÚ?ïâ7†c±^?pÁpƒ'öÂ?mÈyœN¢F?pÁpƒ'ö½?ïÿyJÝ¥?f—¡*ÏR?Ö¤]Kw!?f—¡*Ï64FGL J1346.3-6026¿ÊëÏö]1?ûL'à°«À8q¡ueÀ:¡6¢S|@''•>@-@˜ÿ%­B?°üñ>~–?»B	å²@
ßËâ˜?þªFJ?ïÿÿ" 5•¿Û[gð$–¿ä¶0íÖ¿äù'c€¿èQ
I/û¿éÊßâ©-AGNrdg3FGL J1346.6-6027Cen B?ÝmÀ-Ò?ËÏ79Šu¦?áIéþw?ËÏ79Šu¤?¯×þðc?À$ÒDc4?îò€ùÍ?À$ÒDc4?â!«µÌh?»C%kßì?Û¼¨•Üg1?»C%kßì?ÀöpRx?žº¿ÅŸ2J?ëÂcø«b?žº¿ÅŸ2J4FGL J1347.1-2959¿ï̏˜Ká@?[4ø/Q&À9ûŸÓo~=À<BÙÊQm@æÀ3â/µ?ý"ZÖk®?ºbg÷¶?»à€&(@t G2Ä?þØépq'?散ª?Y?Üg¬Óª7¿ÜxÏ>ìúÀ¿ØÍËz¿åºçÇúÖ¿×`óà·æ6AGNbll3FGL J1346.9-2958NVSS J134706-295840?ïÊä˜Ä8?tåhÐZr?z³ýä ?tåhÐZu?îdÓé"*ý?¹…æGó%Ü?©²Ág½P#?¹…æGó%Ü?ïr¿	©´?Žõ-¦] ?'¾hÊÉ{?Žõ-¦] ?èJV\YÀå?«û×jIl4?ÎÖ¦Ž˜üj?«û×jIl44FGL J1347.4+7309¿Ùˆä•$p@E¯BöÖÀ:øˆҜÀ<ʔøJ)@‰ðP4¡@)}Ý{pº?Å·?ªô²S.?âÍ,n@/†—3bÙ?ï)Œ‹"Y¿å|'€Æcý¿ëϒ_µ¿á¥Ù]ÔÇm¿ïÿü¿ÙŸC?Þ{©Y*=ÁAGNbcuNVSS J134734+731812?ïý¸"'¦º??õ
}jèÎ?2;crÊ+Ú??õ
}jèß?ïøækæ^¨?uøͺ¡_$?LfPf…\Þ?uøͺ¡_%?ïÚÖõþ?t˜@sSq?r"…{ž î?t˜@sSu?ïðƒS7?T³^4?^ùãY'?T³^44FGL J1347.6-3751?äôdk…¦@7¯ŽŸj"óÀ:‡©­
À<ô¬å§@æ#·ë_@[r>á½?º™+"î?É)I¥e·@
£ @¿ä@™!ç±T¡¿€¿^Ð	A?Þë®9cÎÜ¿äßâSFÏ¿äÓsëUN¿êqZ€a¿ïÿl&™Ç½AGNfsrq3FGL J1347.6-3754PMN J1347-3750?îìD{f?ª-y?Øï?®q;¸N©œ?ª-y?Øï?ïöƒiÉÏ?lÛD'ˆu<?Rù-øl`¸?lÛD'ˆu<?ê2C"?°×q8ó(?ǖ6ówð?°×q8ó(?ï«_œÀCd?o•??'?…(Ïï&‹?o•??‡4FGL J1348.9+0756¿½G¢M¬@Pì¿±[WÀ;'/Lô¥YÀ<ŸÀ_@˜@ 6Í.Çhµ@cpÍÈuO?Äái§c†¸?{ó¦‰?¸Å›€#¦Î@°Î‰»U+?ï!
÷9ˆ¿äi;,ü¸M¿Ü4…ãÚ/Œ¿êq¦ é4¿¼am¿\]	¿Á§Â盰AGNbll1RXS J134853.8+075704?ïü‡bLž?9Ã0e1<÷?;Äí›y?9Ã0e1<Ù?ïýý¨mHn?GþK…¸?0¼•¼©?GþK…¨?ï羡
¡Ž?pŽŸßÄéÝ?hA^ò^s"?pŽŸßÄéä?ï÷O<®WÂ?Dðn:†ÁŸ?Qa†£P{X?Dðn:†ÁŠ4FGL J1349.5-7153?íUžì9×'À#¾è»¶À:^qS)rÀÀ;æ"4­†¶@:û³•V@Çc»';?»œ
7;€Š¿³ivRˆŽ?û
6 ¥ý?é8.¿å˚gõ²Ÿ¿áu³Á
&¿ìã4–~\¿×çâT1¿á½'á>sÙ¿ÖFÁ#>AGNbcu3FGL J1348.5-71502MASS J13490974-7152510?ïÑ]´¡šO?~V+V ã?wQ%¯2Ø.?~V+V ã?í[×â¼Xt?ÂUOT½/i?µ!@ê<[?ÂUOT½/i?îr¢çª@Ì?žšÝdDÜ?¨Õх[ó3?žšÝdDÜ?èóQšR®?´.–÷l€?Ì2»ñ–µI?´.–÷l4FGL J1349.5-1131¿Ñóxˆ2th@HnR'ƒÓ_À9Ñ×ΈÀ<Ñqw;¡@gŽiâF@køüÖÔ?±`'?º×ù%Æ83@1ù⯍!@¿¨ƒÂAÙ¿Ùò½'È¿âYLV¿æ¡*òòÑC¿èò™°?ÎL¿éÓÔޔ‡¿ðAGNfsrq3FGL J1349.6-1133PKS 1346-112?ïýëV$¯·?+R,Â,,?0¥Nڂ@X?+R,Â,€µ?ïüãb–?L('"?!é?8äïÿÓF<?L('"?!æ?ï¿3	o¢ä?zeÞâôá?€3=¤G?zeÞâôØ?ïÿ¦ëüþ7>ý0èöÍ;Ü?EÀrO·>ý0èöÍ7†4FGL J1350.8+3033?â}íSøÑ@S#'©"áÀ9¡%t9ŽÀ<xáR•Ï@F•[œ]ï@ÚöƛZd?°%ºç?·'.~SÔ$@f¡aä÷f@"·wP?ÒXÖ%;"ì¿âRñ©ûçm¿ç8⟜é¿äc²¢)5.¿é'ï~R–P¿ïÿÅbu@AGNfsrq3FGL J1350.8+3035B2 1348+30B?ïü¨'Ü?4ৠÅ@ù???š»q!?4ৠÅ@Þ?ïüOž™…Y?RøßN³ý®?=ƒ3Õ.ü?RøßN³ýž?ïÉ ¦cs²?w^U	\Å?{o¬ÎF&'?w^U	\´?ïþb·N¶Ì?ibrH{Ö?)ԋ"9d?ibrH|.4FGL J1351.0+0029?ê]êÇ0Ü@Má;:h±šÀ:d­
ê¤NÀ<jm÷È@¡lÅûø4@âmæÎ?ùY}tË?¹•þÀ¡§?õ%b?8È@vÙÑ4¿Ÿf…Åý$Ù¿ä	•ao1¿æšÔ,<ží¿à¨1ý©
«¿ïþpHgwÞ¿êrÀü§†AGNfsrq3FGL J1351.1+0030PKS 1348+007?ïýïÛ}?,jí6OX¥?0‡?$!À?,jí6OXT?ïüŸ¬wû?Rž%×4C?;œ@'¼?Rž%×4C?ïæ!'
f?olôŸ±â?iñÞ}ò›T?olôŸ±ä?ïý£5—=?#åvº[b'?2æSF«}?#åvº[b¥4FGL J1351.3+1115¿ÏsTu@Q1›€#¦ÎÀ9t™kvp À<
cu^P@…oòbü?ý+þ‹‹º?±@¥\ˆ?°¿ð©Jè@¯\äÝdË@á´¼µ¨n?í°çɨU?¹ðQJöH¿Ü"÷ž\¡ì¿ß"S¼ëƒF¿Ôk•D C¿äM~8C"AGNbll3FGL J1351.4+1115RX J1351.3+1115?ïú솉 ?>MwŸò"]?DMåØ÷~¤?>MwŸò"q?ïùjó i
?`AÍf ›?JT3~[ÚÚ?`AÍf Ÿ?ïã˜%–€0?s"Ø~Ê?lgÚiÏ^?s"Ø~Á?ï}×Q—Œ¯?|.tX_:d?EÍj?|.tX_:b4FGL J1351.4-1529¿ïÿ'y@F|SŸºEÀ:}«fJ·´À<`š¡×U½@­ïõEçÁ@ÃÙß?Á»»?™½)Íó?Û¦£Æ™,@""ì¿ÞB#ßX@¿Èš×‡:òD¿ä1YtœU¿Ù"öd ¾|¿ã\YýL¿Üß齃AGNbll2MASX J13511746-1530155?ïýà">¢?*Ó՟"[?0þïÆ
ÿg?*Ó՟"Ý?ïýf¦Iû£?QO÷üÚ?4ÊÍ°"ä›?QO÷üÞ?ïùu2á['?PWF:f–?J+4z'º?PWF:f¤?ïõÖV˜eù?A4Å?ðڈ?TSRÏ4
÷?A4Å?ðÚo4FGL J1351.7-2912¿Úڒߠµ@?օ3±tÀ:J4ÿ¼
bÀ<.43
s†@³Ç­ËÖ@=•!dԖ?Äab*Âv?Ð0š<+ÕF@	¾È'L@K8P©f?å}d¸|߿߀-·É/‰¿å+¦—㷿噹Å¿ïÿúVrÓ\?ïÿÄ`"AGNbcu3FGL J1351.7-2913PKS 1348-289?ïhƒfн?'Y¿
5?'ü"%è™?'Y¿
8?ïöFQ$=•?qC-}W4?Ss]·"Ôˆ?qC-}W4?ê¯o2¿?ªNà_¬¸?ÅCæC¯5?ªNà_¬º?ï¾²»gQœ?s󹐃~ø?€SQ&+˜ß?s󹐃~ù4FGL J1351.7+5542?éÐäJ@M´¥œ[dÀ;•Ùs¤<‹À=<ÖJ$@ŽššuŒŸ?úŒõ–ðqî?ÒÅ%îÇÉ?ã‡/iz@".C	j@´Äî1!¿Ïì\	@E•¿ïZu%F?ì_Î1PÚä¿×álˆ€Ã¿æSÿ¨Â,¿ïÿøþÙå9AGNbll87GB 135011.8+555656?ïðùV§â¬?bZÿ
Äý?^
R°:¦¨?bZÿ
Äû?ïô²5v?oeö4B?W›"áê?oeö4E?î‹ÇVÐÎ?¢ù2ÃCR!?¯·CŠ'ó
?¢ù2ÃCR"?ï;'ôyh?ŠúïÞ1?˜®pÒô?ŠúïÞ14FGL J1351.9+2847?íKˆdu60@S"T6¸ù±À;' ŒÒáºÀ<î%ÎÆ¢@Š·ÖpŠ?üýŸ‡Ü?ÕËÛø8á?Ìmñ	Â÷a?ø¢³ôŽ²¶?ÿ¿iÒ~¿ï¤«{Cm=?ïëu™àv¿àkTñ¿Ðü¸''ì׿åévP¿5¿ïÿ'R}{AGNbllFIRST J135154.4+285007?ï÷a1Åy:?Påb.—žÕ?Q=œu
‹Ø?Påb.—žÒ?ïì0êºsm?*·Á0–?cÏEŒ"	?*·Á0˜?ï–Å?ƒQ	ëd€?Š|;¸?ƒQ	ëdƒ?îþž2®e?~6ÛWRŠ? Õ¦?~6ÛWRŠ4FGL J1352.7-2742?ӄsᣇ@@œ°À&ÌÀ9ïHk©œFÀ;鼌ã©@‹¥ÝIǟ@M_Âví?ÁlÙ݁zê?ÅPžéd³@é¾àzÿ{@]¤í_¿X¿Õ8~âHN¿èJ€Â2?¿è.ewS¿ë@˜Á­^ó¿ìKt½Âè¿Ù¿†ÞV&AGNbcuPMN J1352-2745?ïÇØÃí´¶?wÂÏþIX'?|ž	%¥ ?wÂÏþIX'?ïúyV'½)?Y¢S¹y¶+?F§aY(?Y¢S¹y¶/?î²ít^Õ ?›ÉiÈh¸?¤Ñ(º¥é?›ÉiÈh·?ï¡ãóP+?rNªhÙ×R?‡‡>ëõ=?rNªhÙ×O4FGL J1353.0-4413?îá™9c¬'@1D^=¢ø¾À9u –
À<ùée‰È@9€H9Ö@cZþSW–?²¹'©gB?°c¥kßÍ?ü6~â^.Š@õ¾]ž@È¿ä«KÞ$ãå¿Öì@Ûgo¿ãýMž"[¿âgT"*d¿äÌ~É3»¿ëZ0Íþ%4AGNbll3FGL J1353.1-4414PKS 1349-439?ïóCñ×Uo?VÆƃ?YxQUÄ?VÆƃ?ï痢ŠÍ
?xªtšE%5?`XZu2ö¯?xªtšE%4?ïÅÓ9ȉ"?€'.¤GLç?}c»6"?€'.¤GLä?ïyÿÕ=y•?{6sځÆ?ÀXPÍ^?{6sځÆ4FGL J1353.2+3740?ìZ»ëqJŸ@RPñýÞ½À:øªÇ¿FÒÀ<ºjÖ7¯š@(YØ8À?þšþSW•é?ÑK,¹œn`?Å<EÖxó?ót1ËT&É@W9°$ö?ïù¿`}™¿ê:'¦.(¿á hUSïk¿ÒgC±Ý¿á¾Ÿ­¯Ñ¿ïÿå=†ô&AGNbllRGB J1353+376?ïÿ_ÞB‰?õ7xÏã:?7¼o°?õ7xÏâº?ïü­°š·L?Râì"½âÀ?:'{*Ešý?Râì"½â£?ïܟÀ§'0?smQûy
O?q°¬lgt?smQûy
V?ïÏáYÉó?cf{éÉ?xwS_?cf{éÅ4FGL J1353.3+1434¿ïÿ©\‹¤N@Q¸«`kz¢À9æÔø³À<e¹@þÍÑ@ !‡å<@üæb I?²˜8_[Éï?TrÈkáqí?¥(æ~#ÇZ@
»Õ§ç»?ïüü_·u£¿ä}üàeÛÒ¿ä,u©ÐH'¿â0›©>R¿äa߃ˆ¶¿éfj˜$N"AGNbll3FGL J1353.2+1435OP 186?ïùÉqê?nPç-Á²?HÚ;»àO(?nPç-Áµ?ïý——["l?J<RÐÙm?3CE#d•¨?J<RÐÙf?ïñ ì~?ac{NW>?]ç¿Â'à?ac{NWF?ïû\'5L?5DSÏS¦?Cª·*Ó¤?5DSÏS¬4FGL J1353.4+5600?æìï'8ën@M…çÀn¹À;A£[º:úÀ<ºŠ´úH0@ä4µê2@‡"ƒ¸†Å?ÃÙ¹"ÆxË¿"šmÚÎî?Ñɋ¤¹]Y@3=gµj¿ïî5'˜Ì?ïíÜ|m8è¿çl]Á|6²¿äXb—¤Í¿àƁŠY5¿Áè›_lw"AGNbllRX J1353.4+5601?ïùÒPw2?NÁÄ=?Kü¶¾#6‰?NÁÄ=$?ïýqvõé?I7™·:å?4wÔHPÀ‡?I7™·:µ?ï˳æà±?},êíjé<?z&§~'?},êíjé3?ïëYç¯7^?Xp>5	±?d¦PÈ¡Ã?Xp>5	±4FGL J1353.6-6640?ÙdYiê.À)×⪄£À9þ…¬|ËÀ;ϏÁàá@ ÅÏþ¨0?þÚvÙ{0ù?¬ï܂ˆ—$?_¤ßʚ1?µEÀÂ}i@Èm`€žK?ïÿwD;Ï¿Ú×.(\¿â³y…'¿à?€³ï†5¿×ȱil«¿Ø"<z¯ž"AGNbll3FGL J1353.5-66401RXS J135341.1-664002?ïøéŸl&­?ENR0
")?LY'OeKš?ENR0
"G?ïüfϒ/?Wúê¯w#?<Ƀn‡¸/?Wúê¯w"?ï'SYǼ×?³(tVöb?k)ŽÊ?³(tVög?ï£âÀ(M\?vÐw$Q;?‡Oõì©?vÐw$Q:4FGL J1353.7-3936¿±/I|'å@5±¶€Z-sÀ;Ȃ—õT«À<ØøγVÚ@"´à®ø{?öĺ|h?Ú&Á HàD?Ú{¤üۈ?úµÄ}î@ø‰*
Àx?£!¼'õ
¿ïü˜!I{Ê?ïþ±¶ÆÑ
¿£×*©»¿Ñ³œ¾ß¤¿Ú€~ÀzYAGNbcuNVSS J135345-393711?ïìÃ9ÖO?jì¢þ~0V?cé<Æ)°Î?jì¢þ~0U?ïûQq-$?cúcÂ?Bº;ïKs?cúcÅ?ïÏ&Úf'?yÖ²Ãmä8?xl'Ìû¿2?yÖ²Ãmä1?ï듄e¤‹?Z1®zԗ?dl{š[ug?Z1®zԗ4FGL J1354.2+6934¿Ö]s±Í~@GJ»˜Çâ'À;9‹n]«­À<⟍Ï`ü@ëëêÊ8É@Ñ·Xâ?ÕlEãäìS?Ó`;^ÐÅÖ?ù|ÙÚÒI?ý€ÌC:?ïû:~+)$¿ç]=B€®¿á¾-,ˆõ¿çiÆ×p•¿ïÓ9ÎWçH¿ï*èáÖIAGNbcu87GB 135252.8+694626?﹐kÍi¹?"7I¸'R?›å¥'x?"7I¸'P?îébýÑN?¯¡{'mêú?¡iÐ"ë?¯¡{'mêú?ìòêò|Ù?¡ÐϝV
?¸h«xl>?¡ÐϝV
?ê"yuƦ\?©…§X*Ņ?Ų(åf'?©…§X*ņ4FGL J1354.3-0206?ï`­†@L‡çB™Ø"À:bÑÜFwÀ<+Z§ƒ@;ç¿ÂMB@\àž:é
?Ғ	†gä?á%'`À48@×WŸúë@¤R˜(U?àÒt¬zFî¿ák™v^+/¿é•1 6ç¿ï¬ÖøŸ¹n?ÚUÛ>T¤r¿îû¶úÓpUAGNfsrqPKS 1351-018?í¢2#›?µ*ðØ
G-?²ï>o†ã.?µ*ðØ
G-?ï÷ÐÃV?½…»K`/8?žáçœuU?½…»K`/7?ådѧq&å?µÈVUɋ?Õ6\±²6?µÈVUɊ?îµ;#&ü¹?¡:fš1sU?¤¬M͐4i?¡:fš1sV4FGL J1354.4+3707¿—í;ô¤[@RWRÁmóùÀ:‡à	Às"À<"Ûá<ÆZ@ãZÅô@"?ÿ¾•·ŒÉ§?¿˜kàè|p?£\Ðeˆšï?ås|>ió@¦IÐÙvÔ¿ÔWQ?ãšÅ?ì¤'D`'¿âƒ''g›ñ¿áÞSÝͦ¿ÜÂ÷¡aº¿à蒀u±2AGNbll3FGL J1354.5+3705NVSS J135426+370654?ïÚ2¡Ñ"Î?pçðá/?ræ¯n˜¨?pçðá/?ïõ¦C§¼"?h"Ï"‹£ý?T³x°†Ø
?h"Ï"‹£ú?ïؐszee?v£[úiï>?s·ÆBÍM?v£[úiï3?ïÂZCÂÅ?‰œÐ_ÿé?ž´·‡§'?‰œÐ_ÿè4FGL J1354.7+0623¿é©ùWC@PøôsÀ;EÖÌ*žÀ<¬Kä ÷@ 1´XÛ?þÐßìdAÉ?×¼.Ääv?¿L'Jò—?ì°ç~~á@†,ÞZi?뛽˨	Ÿ¿ä	"ˆÁB¿à™"º\‡À¿ÐÈøÂI?¿åøžï!‹¿ïÿø]Ê5™AGNbllNVSS J135444+062249?ïþÚ¼3>Ï? ª"
«R?"T<Ìl? ª"
«Y?ïüÓ8*¢?O"f5a&?9f>¯Ê÷6?O"f5a.?ïëͦp¢¹?n±<¶?d2Y]Ff?n±<¶œÿ?ïÔ>ÉÊ?a6㇯Â9?uõà›ó??a6㇯Â34FGL J1354.8-1041?ìÁ벓wä@H•žbV6mÀ9y˜éåÀ;ÿä[^Ëg@n¥ÇzS@*¬azŠ?³Æÿ> 4ú?ǚ}DNc@#»@³Nw@›°´é+R?ºªÅ»ám¿âÈ}}`Þ¿äù— ¢‰¿é[ibš)¿æ1]À¥w¿ç± @Ò®
AGNfsrq3FGL J1355.0-1044PKS 1352-104?ïÝd¡''9?s@qQôM"?qM¯6¾ãÛ?s@qQôM%?ïù/öÙ /?]¦¿ÓV?K@$›DS?]¦¿ÓV‡?îyM3ÖØ?›ËÞ¶¼Å…?¨n»,'i?›ËÞ¶¼Åƒ?ïõ[ÈõR'?CD"å+?UHnZß^?CD"å#4FGL J1356.2-1726¿êV³œ'Ð@E]ȟ@¢‡À;ùÿ4þåÀ=2Pµ$:@ @ԋ2"½?øóy	YÂ?×[	T<˜?íGâb
a-@
VŸ¸g?ýø8RÌ+¿ëÿÝe¡D‰¿ØàEš¾Ý¡¿Â¢HڏX¿°¹€AS²¿êêË»TÕD¿ðAGNagnPKS B1353-171?ê"v›ZD	?¿ˆGòŒÅ¦?Å®%'–ïÜ?¿ˆGòŒÅ¦?çÂíҀ|ý?ѱhK]?Ðz$Zÿ?ѱhK]?å2ƒ!¿‹Ë?ºu·)½†?՚ù¼€èj?ºu·)½†?Üô*›´±Y?»¸O³þ¶½?á…ê²%§T?»¸O³þ¶½4FGL J1357.1+1921¿îÒ[Ìûó@RBä¸{ÜðÀ:?
€Œ'ZÀ<^gpQ¢@‹íi>]@ý‹{ɤú?¼¸•!(³l?Ž3Š4æ€l?Ç⧋P@
6҇v×M¿ãv֋'oڿ䜝Öj/¿ë SÇþ0ó¿åèe¯‡A¨¿ð?ðAGNfsrq4C +19.44?ïÿ(±ú? °iU™g?úéÀ¼¹`? °iU™m?ïýӘ	݊?LG< ›C?1c?±­
?LG< ›N?ïߏ/óº?r &¢NäŠ?p8hu£-?r &¢NäŽ?ïýOÍþ>?-—K
}?5ÎŒ?-—K
}k4FGL J1357.5+0127¿ÓŸ2üZ‹K@Méä¼­šØÀ:/½¦îíÀ<V8‰´IH@Ú;ƒd@ü wnÌ?Àx^ õ-"?Ã%›Åî·@oPóÇ
?ÿî>¯h7ø¿ëïþ€#&?ï	þ¡[.û¿ãOˆžŸ'Ø¿ä‰]aZ
¿âàsr¾c}¿ïÿªÅÝðAGNbll3FGL J1357.5+0125RX J1357.6+0128?îòì"T­?¡o˜VÒ/? Þa6ºµ*?¡o˜VÒ/?î#î}5?ÀZQ»''P?­Î,®ª?ÀZQ»''P?íü§ýY'ƒ?¡{¯$¾W?°À3kð?¡{¯$¾X?æ›\£'¤?¸OÜå3W?ÒÉFä¹°·?¸OÜå3W4FGL J1358.1+7642?ÉLÅ"ɋT@CãŒCoÁYÀ:ítãìÀ<¯¾5ZTà@ŠÍ©ìx@¤%t:?´,Ù&ø?¦ÒU¢ÉÄ?ðjâF±•9@wûmŸÙ?å_¢!¨q¿ß›j$ÎA¿äýýâŽl¿ãÙwÕúrø¿êþMxX×2¿ïÿŒýÿʦAGNfsrq3FGL J1357.6+7643S5 1357+76?ïùå'cP??B$ép¡½?Hkbr¿ò?B$ép¡½?ïý^Ÿ\Xõ?Ik®é‹?58[
?Ik®é"?ïÀY2˾î?€dy†Þº?Ófš ˆÆ?€dy†Þº?ïüG†â.Þ?,»«ÉŠ[õ?=ÃÈî‰í?,»«ÉŠ[â4FGL J1358.9-0703¿àò$xF@J
At>–>À;Ž²‹Øæ·À=þæ$Œ§@&þTb`?ù(
Jk^?×ÉÔ_hEd?çN—rwì¡@Æþ÷ÂCÝ@mI%7òá?ï­àx{;á¿èÈ¿AHõ'¿Æj!´Û"¿Ä³w¼$3¿íQÖ¤¿ì‰pÃõ8AGNbcuNVSS J135850-070403?îJÖFÈ?®ŽJóó,?«Ržî;"Š?®ŽJóó,?~¥'¶?¤Ît®w?ŽàV›Rà?¤Ît®w?êS.··š?±‹ØÕW»?ƳE!#—?±‹ØÕW»?ë#]ó(ËX?®gûË[ÞÍ?Ãrˆ3\ҝ?®gûË[ÞÍ4FGL J1359.1+5544¿æätÝ+^v@Mq%F
¦LÀ9¢x>Õþ¥À<Q¸ÕŸf@v$4Õk@ã¼ûžqp?­7¿^û
'?¼û•0©@@c¦@q	@Å?à?Æ?¿Ô÷íwg?ª¿ã=]º¿ä<Ž@ @¿è«þ +ï¿ì ©¡Nš¿ßáŒAÂB/AGNfsrq3FGL J1359.0+554487GB 135720.6+555936?ïô¦$
¥-?Ság"Ù^ã?V³·êµ¨÷?Ság"Ù^ë?ï÷o©Ôâ?^ÿ'PÇ?Q!ʬV;ú?^ÿ'P¹?îÓ±yC
F?˜'V
þ?¢ÄèkÏ[˜?˜'V
ÿ?ïÃ"M!?h]ü­J*?~z=Ùuï#?h]ü­J*4FGL J1359.1-1152?ÔOp³}Ý«@GՊ"-QrÀ;ًŸeÀ<ÏÅ'iú@#"ß³Y^@?çK¶ý'¢1?æZŸRk2?ã÷{a .?øȃweR@ùi'é÷Ö?ïñZJÏ1¿ÍÏã؂µ¿ãßIÈ¿äøRAkZA¿ÿâm•Q?ÊxýrñºAGNbcu2MASS J13592131-1150440?ïÒfáÎ~?Lh¯ >?v̏ýÁ ?Lh¯ >?ïû'´
Þ2?]Gézœ]?Aµ/ȇ4ý?]Gézœl?îÉLXwt?–O°¹x?£k:xØÄ?–O°¹u?ïáH%Æ?Î?u´™"â¯@?n·Ú9À1ù?u´™"â¯?4FGL J1359.4+0202?ì<'
ÍWÍ@N'¼U†DÀ:"R:_w_À<Qhª
…@ ¿'țæ@]¨!ò™?Ëæ	³õ?Ï؎!yd@¿2½ÂmÎ@Z½Ä³Ï?ïÎÃè!¼é¿ä…Õ"ܤ¿çuM‰öŽ¿áÉ/ß@¾¿ïÿ×,uª?æ9i"ƒb¡AGNfsrq3FGL J1359.2+0204PKS 1356+022?ïï±G««I?a—'qÄv£?`N¸TT·8?a—'qÄv£?ïûeoŒz·?SÑ$±›ë?BjAÎ K?SÑ$±›í?î'2£»ð?–ì¨^‡–?¦ìÓÕÄA?–ì¨^‡–?ïׯ{Qåî?d/íä?t(BW
?d/íê4FGL J1359.7+4012¿…ø͟|Ò@Q°–»™À:V²w¶ðÂÀ<|J{NTø@^VòU'@ž[BEõ®?ÂZCBð?О饴¦@	<J@•òE@G,íHî0?ï÷6Íòfº¿Ù«"}¨¢K¿è>Æ¿—…¿ê~€¿ê'•¿¿ïü€s,óAGNfsrq87GB 135731.7+402612?ï½Ð©
Ó?ƒ·åäïO?€‹ýÕ½Jð?ƒ·åäïN?ïùBßÂð_?_I+Å«[]?Jô€ô>…e?_I+Å«[f?ì­{ü¥D ?£wÿ¡ôK`?º" Õß?£wÿ¡ôKb?ï»BhK¿à?o ü£I¨?/eíE?o ü£I¬4FGL J1359.8-3746¿îÀÞÿ¡«£@7&=_ÜßjÀ9…/…(ÉÀ<¨a³y@ºYÀ7@"ý°šg?¬ªþå´á¿ 3ÀîÈ?ó@YÂ5g@N}âÝ?â{8 Z}û¿àr·!ê¶m¿årÚ/­m¿Úx›)ñì¿ÚÄGÃ
0j¿åÅYa›AGNbll3FGL J1359.9-3746PMN J1359-3746?ïû雃{~?6îø~BX?@Y'òÐ?6îø~B]?ïýµ‡HY<?GôhçݏÌ?2SŽ6$ó?GôhçݏÀ?ïõ¼«/…?dJÚøIº?UȆ© ö¨?dJÚøIº·?ïó€\õ$Õ?F0^%"?XÿF¶UŠ?F0^%š4FGL J1400.2-4010¿í¤ÃÓáx{@4Ðù;À oÀ;ñ՚ѨÀ<Š¹æ@;Y@ ÐXz•rn?ÿ"<jÿR?ÉèxyäG"?³ÿè¿,âG?ä¢ÿñ?ïäOþ΅<¿Ø—"{ªñ0¿Úki¦Wî?ÞçÖyô¹¿äh M¼¿Úd¢Qy¿á'Y
]QAGNbll2MASS J14002208-4008235?ïùÛ2Â?UxSfp?H"7›èõ?UxSfp{?ï	«û¯?¢Tw'Ž˜¾?½•?ƒ?¢Tw'Ž˜¾?ïÁA"Ìú>?~PçÝr3?_n™'àµ?~PçÝr(?í(øÚ?¢´ìI›I?·v¸?/>?¢´ìI›I4FGL J1400.6-5605¿°;hÆŠ@õ†_*2À9 syt`$À;¥›/›Ï@§ÍŸ°‰ö@
œ \–Ú?µ@1ôCß(?·\<ìÅe¥@,Gõb@i‡-0e?ïÿúŒ—Ó¿å:ú!™­¼¿è.[}T>œ¿äǸ@MÍé¿åyÁg‰&¿ïÿܞüÚÝAGNbcu3FGL J1400.7-5605PMN J1400-5605?ïý‡ÜJñf?>{K†ý7?3Á¨tÊÙ?>{K†ý7?ï÷&uo§'?j¡Å`F?Q³ ±¯Î?j¡Å`??ï™A'w¾?"^֍‹±?‰¯º¶"a?"^֍‹¯?ï갏y@?Pų"&eÅ?eOp†¿ì?Pų"&e¹4FGL J1401.1-3717¿èue$Óp@7†Qm°ÝƒÀ:ˆWUQk-À<T"ÿ®¡i@ ÆK¢ë§Ù?ýJm\#íE?ѽH WÎÉ?»®ÛJ>´?ìÆÝ¿¹=ú@©ùŸ"®ž¿äp]€c½•¿äÐvH¿æ•§œ'œ¿È/Š1FÉé¿Ýê …0«ï¿âÞë}'üAGNbcuNVSS J140113-371757?ïüŒZøýÊ?4Åi"ÀuË?;(8¤©?4Åi"Àu°?ïý+3ðxÒ?PË=4•æ?6¦`|9l±?PË=4•ã?ïì8.?s©®k[Ç?cÇr€æÐñ?s©®k[Ê?ïÔñ­Ü?d!!ù
?uòÀ)ë?d!!ù4FGL J1401.2-0915¿í°òü_@Hïâ£Î¦ÂÀ:¢nÚ©.bÀ<''¤{u@Í>¿‰È?ÿæ҂s"?ƪ4Üօ2?ɗ(¦w!?þó(ýOL@ë8[犿ìî`e›eL?ï÷`Æu¿äò–UAzõ¿ÜPj{žÝ¿ë±Èd?¹w?§ŠÈñAGNfsrqPKS B1358-090?îŽÚܙñ?£/SÌùàR?§R6`îo?£/SÌùàR?ïñ|RÏÞK?uÆ?›RØ?]Z`Cm+?uÆ?›RØ?í³‡iq?¢à'íÀ?²gCnj´y?¢à'íÀ?îæCýج?Žßœï!nÅ?¡›À"u?I?Žßœï!nÅ4FGL J1402.5-1827?Û?
#¥–@D¡¥q"À:($5inYÀ<(]yWÚ²@
«)¹ã@·Mú^ÖO?½¢³ôŽ²¶?rõoÇýÊ?°öÌz—uÓ@¼"K̲ ?ì×aPQý¿æŽÛʖ'¿ã˜íl…¿çŌÁïÏ¿ïÿþó…õ?ïÿÚ €AGNbcuPMN J1402-1825?ïÞÛ²!I×?t›8sÇ®õ?p'&ï[†?t›8sÇ®ó?ïú Q'Ø<?c;pgíd?G~¹´Ÿ?c;pgíd?ïDiôÏ¾?'´QÛèM?—rÁnF!?'´QÛèK?ïÏéíä½/?k±D*34?x	
¡g'?k±D*354FGL J1402.6+1600¿ë<aÿ)S@Q†	€²BÀ;-Ãք´À<­póˆ"@ …H~Éà?ÿj`Æê4½?Æx"%çEI¿{)øã0Zt?´¹øå¬Ã@™'6¿ïÿçÁŲ§?ïÿÿ>¹ú¿ëbrϏ¿ÅÚñéû%¿Õ0ÿ;ßÕ¿ç£ìòù‡AGNbll4C +16.39?ïÿ9QÔtÎ?SŠ` Ï3?ÕÅqf!¤?SŠ` Τ?ïþ7øû?Fš'ÜlÙ%?,€pOªï?Fš'ÜlÙ?ïÌÎþFÕB?€",B¡Hd?y˜€Ü•^ÿ?€",B¡H`?ïûœr5À?8nû{|?CùŽ7)B?8nû{|'4FGL J1402.6-3330?äŽêžR?@;GÜ7£ÛÀ:˜) ã9÷À<kiA@®[®ýY@:9Å«â?Ò¸µ¾"N&?ïj-›C¾@	¼=h@[:@1mD&¤?f¾uœ¿¨»¶OùC¿î!3âÂ]¿â$A"HFÁ¿ïÿ••_x?ìѹÁ,Z§AGNfsrqPMN J1402-3334?îv÷ÂÝ[?±}$»µ[?¨ƒß2*S?±}$»µ[?❜>
¯É?ÕEƒT·xù?ÚÄǃê q?ÕEƒT·xù?ê2×Â)¦?°ÃÈ΍?Ç4 ÷[g?°ÃÈ΍?á+y­\w?Áóóé!¸?Ý©¥Gð?Áóóé!¸4FGL J1403.4+4319¿æN©‹üzŠ@Q
ðoiDgÀ<#01 3|À=$P%"õ@"…–VÄ?÷"Âkðê?×û .y?ÍЛ¹Y}u?ù´@€#@¼&‹*‡¿ïÿý{ÁA~¿ïÿÞ°ô)?ð¿âH+üÆ¿ÂDm'ºZ¿Âd5^±'2AGNbllNVSS J140319+432018?ïú÷
A¶Ú?PΜ܌×?D#Öù$"s?PΜ܌â?ïý!‰?z?PÀt/?S?6ó¶/Žr?PÀt/?a?ï"&QÛ-×?ˆsä©Ã¦0?Šök‰4Š=?ˆsä©Ã¦4?ïøÜý…?HP
….È$?Oď°	ç:?HP
….È)4FGL J1404.8+6554¿œËÄ\˜@HÇé·¿ŽÀ:ªøf®‹À<Ž~(א@>Â?Ö?ýÕ%t-Ï?³š³Êó-à?«Æ¥bÇí·?ö7yU@
uèúÕÉ¡?ï÷€—9î¿á"†?IÁë¿ÙŸ:":½k¿Ü‹‰`'eC¿ás°0´Ó²¿Ùl#"¯¥AGNbll3FGL J1404.8+6554NVSS J140450+655428?ïþÆlüo?/é9½?#™09ž°?/é9¼"?ïü†ÈÆ܍?QÅZäË*è?;ɹÉ›ì?QÅZäË*à?ï÷üKësd?`‹É;¾V?Ph)7
?`‹É;¾Z?ïø`âsÝþ?7ªD§-?N|v0ˆÎ?7ªD§P4FGL J1404.8+0402¿ãZ[@N€ƒ§ŸíÀ9éF¹!õÀ<MÁ}ä1@…$1–¬@b"òB¨?³pbé"='?ƒ\³VGú?Ò'!,öX@Qî4P"˜?ïÂ.]á\§¿Ž¬)ò N¿æù­5WС¿Ò=ÉD6·¿æá	/Sª¢¿ÒºBUeAGNbll3FGL J1404.8+0401MS 1402.3+0416?ïõŠø¿:_?QC xì‡?TꁋCS?QC xìŒ?ïû{2C¨1?VX¼¬B?B6ñ_A³?VX¼¬D?ïï0°àø?eÿK—«Ìk?`ÏObw?eÿK—«ÌW?ïÎþ''ñF?fR¨vøñ?x€·6‡\g?fR¨vøñ4FGL J1405.3-0640?ì
Қ‹¿@IàU!š"{À:ð¢nTqqÀ<…e®°'@qÛ$(~N@…ŽêéîF?ΠiA#?½ÆŠdó¹?ñ$lü'œþ@tP+çd~?áC"Lx?ïëقgÎÆ¿êÑ¥CñÇX¿ÇJ|ùzÖ¿æä_æo‹¿ïÿ'Q¦»ÁAGNbcuNVSS J140504-064056?ïîÇ7õÇÞ?b~èˆx_?a8È
8!†?b~èˆxZ?ïÞ¸[ôP?†¤YEr6?p£Ò×ö-?†¤YEr5?ﶫÁe‰'?~	X+¦¦?'U¦Ÿz?~	X+¦˜?î‡y}gë?•&á"Öâ?§Ž¨h)d?•&á"Öâ4FGL J1406.1-2508¿ïÿ²SÇ÷e@A[¾ãÕýÎÀ:Û»}0À<Vºlwø_@,¾yø¿?ÿ–Ù æ?¹'ßV?³RæVáŽ?ùˆ
%ð@
¤íÛ:MÚ¿ïÿ'¥4?ïÿÙiÍy¿ÚÜÜåHĕ¿ÜˆÖž椿æob¬c¿Ö§ayWAGNbll3FGL J1406.0-2508NVSS J140609-250808?ïÿ¡N(d?c‰ñE£V?«Ö:óÆØ?c‰ñE¢Ú?ïûêÖ\:ã?XZ8,?@T¦zM?XZ8"?ïâò(×î?u÷¯SÍ<Y?m
×ê(å?u÷¯SÍ<V?ïáAU©[?`!Z(¬ó–?nû¾ªV¤?`!Z(¬ó4FGL J1406.4-1654?åùgÿA´@E,ÔV.	ÿÀ:à翗Z$À<eôA…ÜM@v‰Á_[Z@_±@L?Ææb H¤?%U`?ìæ?ÇåTƒ™@퇂k?àM³¿ÞIMü¸!ð¿à+bùÌ	¿éD5囹¿ã»gêÊ䕿Ë58›ýÌõAGNbcuNVSS J140638-164954?ïöª‰?7?Lã/Ví·Â?R«Ú큒Ú?Lã/Ví·È?ïý)è¹Ä?O6ý+Ã×?6°º7ÐÍ?O6ý+Ãù?ïÂ.ÐÓïþ?€ƒzjÖ ÿ?~藖¦?€ƒzjÖ¡?ïëùæ9´?QM)	 ÖF?déÆL'?QM)	 ÖH4FGL J1406.6-3934¿Þ± ‡²N`@5z9'ÍÀ;2Êo${
À<œ!Äuæ@#14…×b?óòPµû?Ö|¦Ä¥`ø?ÜL³aì¯@ß덂4"@
^6¬j—¿ç‰Ò¡ÍðŽ¿ç/<B¦¿æ`ï. ¤»?Í#£×dÖ¿")xc,äԿϊ"=fèÂAGNbll1RXS J140630.3-393508?ïýG­Å`é?9Úà©?5'Ôø¾¾?9Úà© ?ïüéótî?VkØž¥??h°dXŒ?VkØžŸ?ï¿ÇϜé?€ø­¬Bú?€ú…¸?€ø­¬Bý?ïüÖÁHJ?5¢º»ˆôÆ?9Iõ½¯2x?5¢º»ˆôÒ4FGL J1406.9+1643?ïÈýŒñ@QjŸDÔEÀ:·í£ùoÀ<'"ͧ¾ @ ÔÇOŠVÜ?øÒó*öN?˅'òP¶?Ì£f÷ÛÄ6@³Þ¿=˜@³ã»¦´µ?ïÜÛ7ɚé¿â} _žû¿º¢>?¿Ðºèß'q¿ÛdóiÅ¿äF a3÷AGNbll3FGL J1406.6+1644RBS 1350?ïýÒ+ÒñU?0ŗd8c[?1n¡huV"?0ŗd8cF?ïùzU-!?]V"H£™?J«¿KyF?]V"H£¥?ï¶ýÈ\<?jjzÿC?'@èù±>?jjzÿ>?ï¢ù
}u?q(NýÁ÷P?‡A¼»à¢T?q(NýÁ÷Q4FGL J1407.5-2706¿ì´Iס½|@@a輜$À;oŽXøÀ<¨¼ÆÅKÏ@!jÑF"@Hpa'ëO?¡6›óf¿º'ê?Nt'?ù"ÿü¥?ýôc>¾­?±f£M!›Ü¿î苤äPw¿×0ÄÃéÏ<¿×êäûAÕ7¿Õá!îgQH¿ÇÚÄ\:éAGNbllESO 140425-2655.2?ïö¥÷q?N$äkëã?R´ûË?N$äkëô?ïóM£Îh?'ÇIÁÐ!2?Yd¹Üc0¼?'ÇIÁÐ!4?ïï´Mâ?k"ÆUw'?`øK²ü?k"ÆUw'è?ïœîã/_i?xÁ`Êës»?ˆÄG4(%×?xÁ`ÊësÀ4FGL J1407.6-4301¿ï¬Ïçñ@1°§¨PÀ:Êõ\8À<B¾Ü-"@ߗ mˆÅ@Vç_ö	Ý?º‰ 'RTa?®`ÈAͪÃ?ò$ötfj@)¼=]ƒ"?ïÍ€°ên¿×.¡S!e¿ßÁf<J7¿á›·¡Aƒ®¿á'€ãÀ.Y¿ç*`Æê4½AGNbll3FGL J1407.7-4256SUMSS J140739-430231?ïý[»z?R?4àW¸hï?5"$.rÐ?4àW¸hö?ïû®v† ?Xí²¨n?AF%瀊?Xí²¨j?ïðùú'4ƒ?e/±'†}?^±–ù<?e/±'†}$?ïü7"ý4M?.#╚Л?>CØ]"O?.#╚Ц4FGL J1408.9-0751?äAó9igz@I%ñà'Œ7À8³çïhHÀ;Ls¿ë<ú@ÒèŦ¾@¦Ós¯û?¨g^«Sx?²ßß#;™^@	™>›A:@›¯|¿©Ý!-ÍË¿áFvÜÖ/L¿å¦@q	W˜¿å
ñú´g¿æºy
2ª¿ëyÍ¡^	 AGNfsrq3FGL J1408.8-0751PKS B1406-076?ïù/pq†?Gæßý•§?KCî>9åÊ?Gæßý•§?ïû³ðÏå?Rþ`/û?A0<àp?Rþ`/û?ï´gÞIWD?€Gðcƒ
Î?'æmª.é?€Gðcƒ
Ï?ïü Íö5u?.³µ°‹?>ùNTNq?.³µ°Š•4FGL J1410.1+0202¿ç¯nPìtw@MO@Än&À9Ób ß9À<V/Ñ|_@ÖC€Þ6Ø@óò
s÷I?¶ôN›ï_I?· Täl|?ÿ‹…L»@
ùÇÚñS?׀ät^Í¿å)B™'¿ãï°A{ËR¿Þ{†^(P¿ìèné¦ٿïÿõ4ÊãAGNbllPKS 1407+022?ïõ0²Ô?PÀÌÔh?Už›ðWã?PÀÌÔg?ïúÚ{·?XfºRþ?D–‡¥$?XfºRþ÷?ï™|ó?Š8'Œóρ?‰ üxƒ>;?Š8'ŒóÏ}?ï×{Ž'ø?`Úwn?tvB8¶ƒÇ?`Úwn4FGL J1410.3+1438¿í¿fR›¹@Pòy»­À˜À:aps/¢…À<[IŽ¿@Vp–ëêI@ߢ'g?Àe@ ¬s?¼ÂSL-U#?ýPÕ©²ì@`dÚEÀ?àý®(`q¿Ë¬Þð»¿^¿áƒþÿyó¿á¥?à?Æ?¿âlÁâ
&¿ç€[AGNbllNVSS J141028+143841?ïҁq¯fÂ?wrþðø‰"?v¿G(Lž‡?wrþðø‰#?ïó$ÍAå?j6€ݗ?XŶe|8º?j6€ݜ?ï¿íc13º?`©GC`?€§3³1?`©GC`?µBô?Y-"Yï®?¥Vd«Ð¿¹?Y-"Yï®4FGL J1410.3+6058?ïå;ӌ%@JÏäy'¼VÀ;ø|²F+À=* ë2¢@"o±UÍè?õf|¡;N‹?ÙS¸ä¸{Ý?˧À£ÉžD?ó0Ì5Î&@‡¦<•1«?ïþ—Ô¿ïö({ILz?éÙl€OF¿±R á·j¿Ò|ˆÛ—¿Á7»˜œïdAGNbllRX J1410.5+6100?ïÿÖc9>úEð¡è>ôÎw¿cžP>úEð¥?ïüâŽk]£?R¨äŽû?8댥ê]?R¨äŽû?ï׃iñ+H?zbgˆþ4?t>Kj[ï?zbgˆþ>?ïþ%´²k?#à™4üÁR?-¤´ÙN*»?#à™4üÀö4FGL J1410.4+2820¿é[hdCÂ@RÿCAžÀ:•ÝÞmAÀ<£xOYÚ@ï£ö¿ºk@
·Üz¿º?ÂpPJUl?»œzŸƒh€?øÂ^™éJ²@#JæX9?•"|¯‡¿Ôs£eË5ô¿ßéIDÂ|½¿Þ'G۶ʂ¿æ3OîTÜÑ¿ï´
ɇïAGNbll3FGL J1410.4+2821RX J1410.4+2821?ïù¼InîÞ?Jbžûœp?IÚDD…Í?Jbžûœp	?ïü¸Ré=?S^PMrX??=h¶š?S^PMrc?ïä÷ϹYT?t_aw"Ï?k0F¦«ä?t_aw"Ï?ï¦i?pÝ­=Æ?†~xz在?pÝ­=È4FGL J1410.5+6215?ÛÚCþÞ@J@8ÅCÀ;k
Çhß½À<»§œ'›ž@ŠK—Øú-@47yéÑ?Áe»È®¿º·¢™œ?ûz	Ì1œZ@´)Q.?ïÿƒVR¿çÞQ"'¿ãŒÝÞíᚿåÉ3 @|È¿ßÐÜH*¿Ò/ºÏÊ-AGNbcuTXS 1409+625?ïóYþÆ?Z@µ¢¶ù£?YLxóûÊ?Z@µ¢¶ùž?ïÑÛ½UÐ&?tó*?w!Uí'?tó*?ï;ë6rþ?'Lßêü?˜'y1 F?'Lßêú?ï•1ÙQ¶^?~Z7ý?Š³‰«'h÷?~Z7ý
4FGL J1411.5-0723¿à'ÀÎàí@I3ÞÑ·À:ŸÆh.½ƒÀ<]ùú,h@ ó¿ÕÃk@0«Ü'<®?Á¶f2¿©b_¤3@?æùžßY—?÷Z®Fú»H?ä¥+"˜†I¿§Ež€ð;£¿åø}àU•´¿Ý3žÞ'>¿æ"1l"Ž?"bèyóÙNAGNbll3FGL J1411.4-0724NVSS J141133-072252?ïÆòAµ¯?vCE3ôÍÔ?|†ß¥(Â?vCE3ôÍÔ?ïE…Òa'?¨'»?ßø?—OE³Ûv?¨'»?ßø?ïÏB™"<¥?{)íö?x^³=á­ó?{)íì?ìG¿\?¡½Ž_¶ŒP?»…ÂÇv?¡½Ž_¶ŒQ4FGL J1411.8+5249¿æ§ù!ø@N!uŽ!–SÀ:ÎÜيJqÀ<ÐÒE²'¸@mòGۋ×@'åp1Á?¹ù⯍ 応Oò†qã?â¸îÞðeÙ@
©3)ƒ?ïZTª|?ì¿ä¢ŸÒ˜¾¨¿ÞíC÷Ò¿è~bÁ–7å¿Ì¸éÖrèÖ¿Úa€Îq"AGNbll3FGL J1412.0+5249SBS 1410+530?ïþ	&ü,+?)@]ÿN?/m==K?)@]ÿN@?ïý¿ÝÀ±?L)笴?2ÿòt˜?L)笴?ïîutááK?h^øÑئœ?aŠ‹³þ?h^øÑئ¬?ïüéô?ÀG?*·xS)?8°^ýÈ:?*·xRÆ4FGL J1412.0+3836¿ïù,W Ï@Qg¸d"À;†2´ˆ2À<Ž#â]@ ˆÂ%ÔÐÒ?û´{'G–?ÉgöHòL?½ËPËÊnN?öÄçûý<@ì$+#¿ïÿìêy…þ?ïùàÌ^¿Ö ³Ô®C¿Úf÷~0ˆ¿×>?©c;¿èr'~túÿAGNbcuFIRST J141208.2+383521?ïÿ§×'?	yŸШò?
 ~$Õ?	yŸЩz?ïü¼<-ˆœ?R5¹c8 ?:"»?R5¹c8?ïì‹BÒ´É?o§ï–Tí?ct½-K7.?o§ï–Tí›?ïð2ÙÛð@?NÜV¨"là?_šLHò?NÜV¨"lá4FGL J1412.1+7427¿íj['³ÐX@DÆ	VÀÖõÀ:¢!óoÏÀ<£èì¾Ü@}s±¨"@‰Ÿ
vá?ºüg>ÀZ?˜Ð—e?}w?Þx~a.ï@­{£ºZ?ÚÙéëÁ"š¿ç E…EO¿âªÜí¬@e¿àyÊÇ9¿èŸú¦ú«,¿Øx' Ï-zAGNbllGB6 J1411+7424?ïîÝ(dMO?[¹¦†<:?a"כ²¯K?[¹¦†<:?ïýÚÃ?R˜=âU?79/IñÁ?R˜=âN?ïâ–^Ú?uñÞ+ž¦3?mçió¡%¸?uñÞ+ž¦7?ïâjŽI]~?Wæ0ìÒ(K?m•q¶¢ç?Wæ0ìÒ(J4FGL J1412.9+5018?îŒ}~W­Z@OHƒýP"À:õênžCMÀ<²Àsøö!@ê²:O\4@SÌÐþŠµ?蛢Íu¿]Ô³tV×?˜¥w¦Þ.R@	J«GA1¿¦À"üêæ¿èh'Zà÷&¿åBl"4X¿è…y¼"€-¿éKV?§¶¿ïÿ[•R<AGNbcuSDSS J141302.28+501927.4?ïþ'
áÒ	?,á0˜¢?-!â߃b?,á0˜°?ïý¬)T¢V?K})Ϻ?2žµZíLÆ?K})϶?ïåP[,\?l­z03âb?j¯¤þÓ¤ã?l­z03â_?ïøï.ÝF¶?;"¥°°Wä?LCDŠå&ÿ?;"¥°°Wå4FGL J1413.1-6519¿îu=f‹ÒÀiØá®aÀ9»1'À8jÀ;'™,ŒP@ۓÜ@]=@ý"$½N«?¼2sÓÝ?™æÇþ9‰í?à.ßFL¬@V†PÀb¿îæÉbµþ?ï"2¼ë®9¿ãbà՘Mi¿á™óÇ™k¿æ)'@¶©¿â"¬Ø:¿AGNsey3FGL J1413.2-6518Circinus galaxy?ïĚîi_?-NÕÃJ?}²ˆñËQ?-NÕÃH?ïú–j ¤?q£9
"]W?Gõ¦U}nÜ?q£9
"]X?îüö8èz?š$MVáS? 0œqx^e?š$MVáW?ïƒõ¼'î?'h#¨«Ó0?þ_D«?'h#¨«Ó/4FGL J1415.5+4830¿ïÑDôäÃ@O~Ü~ñxÀ9¦tÿ†À<K'5!Iý@Á½CÚu?þDv×ͱÏ?¯z4ú]©©?©ÎЁ6ï?ú#ÝTÚLè@Âƒó•¿åMðMÛU¿à"œÚ–¹ë¿Ýý±¼P'á¿Ýš¿]οà™xa"·¿Þòky˞AGNbll3FGL J1415.2+4832RX J1415.5+4830?ïÿx•l2?ó»!‰Ž?í]y¼Ž?ó»!‡?ïü®Šxcø?R–$X–8š?:‹¬<àF(?R–$X–8«?ïô­ÝÖãô?bBb…ý©®?V¤DR8(?bBb…ý©?ïÿÄõ>á4>ñJ7éC×>ý…`fÄ>ñJ7éB†4FGL J1415.9-1002¿°9©ü"Ø@GǤô^À;Ep÷¹àaÀ<Ù¤?åÉ@ÿ0,#@SPÊï?׿-BÖ¿?ïÿþBe«+@"ÚųÔ@¿?Æi†¿ãÍÍlê?Ѻ(»
,ª¿æÁ|^¿ïþaßîé?Üè=)T¿ï^-ôAGNfsrq3FGL J1415.0-1001PKS B1412-096?ï ›ÕtÊ?–ÄÂá¥Àã?‡þÙ
¢Í"?–ÄÂá¥Àä?î÷©ª¸Ø(?º‰hr2? …eTr}˜?º‰hr2?ëOáÁ?ªÅx¸K
?ÂÀxùËë¹?ªÅx¸K?ìÛv÷¼?´»«m>¿p?»Y$HB*?´»«m>¿o4FGL J1416.1+1320¿ä±ó³-|Æ@PyÛ
Ø0À9ÈÔ¨c`øÀ<X¼ˆ±êÉ@*ËâA(>@*ÈE~R?·h_ºÐ í?Áq}ÝÑØ@¹Ç¼Â"Ž@
{NÀWs"?îB # –x¿ãñãr*¿Ç¿äQ…¦ž¿çÕj*@Ej¿ã×MŸ7¿ðAGNbcu3FGL J1416.0+1325PKS B1413+135?ï÷EÚsí?RºŸl¤x?QtKé(&?RºŸl¤x?ïøˆ#ñ?bCèdJ?MßsÐ;Às?bCèdJ?ﰞùæ"à?|øZ›a?ƒØA†ZÇÆ?|øZ›R?ï¥ßI)ï??rñá1X]?†ˆ-µ"0X?rñá1X\4FGL J1416.1-2417?ï\R5óš@ATïܜM©À:—#	¼AÀ<e¤m í@ ÑD€bï?ûI
Öק?ÃpÁÂ؂?Ãî•ç2@&º «q@
	œºá<ñ?çžX°›=ß¿ïýf],+?ïæ¥á{…‡¿Ô¯–[ ¸¿á·¾þX
-¿áåàš	+AGNbll3FGL J1416.1-2417NVSS J141612-241812?ïþ;¿L`ú?',—«2µ¼?,D9ðY?',—«2µ"?ïüßÖ||î?Pð0¥ ÷?9L™¢?Pð0¥¡?ïæÜõV	?q½j`ñî?i#
©öîs?q½j`ñí?ïçîÿl}?ZÌZ{Øæm?h"þƒ?ZÌZ{Øæz4FGL J1417.9+4613?Úàïg}Ä@P§Ú¤ü¤À:ö¤}"jŽÀ<£QùÇכ@^"JÊÿm@ç#? )?ÆhŠ'¾Ú¿ž"$\"7/?є¨½õo@¬Y=ÞÝÆ?ï¿á—_,¶¿å¶XKñp¿ëÐ÷Ÿnd¿ëñõáõS¿ïìu߀-¸¿ïè(‰ŒAGNfsrq4C +46.29?ïþƖú2…?)ë6ÐoU?#–\םß?)ë6ÐoTå?ïóí"Ý¿?oícFŒ?X%âØDQ?oícFŽ?ïÜÿ\Á¹?pNkû¸Væ?q€Qô"í?pNkû¸Vß?ïáû[èt?bÔ^8îÁ?n÷¤‹£?bÔ^8î½4FGL J1417.9+2543¿äÖUÛëoä@Q¦W>«6zÀ:l–ç7²À<N1©Æ7‡@"Ô˄£=\?õ˜¡Ú°»?Àh3›
-?½âËfÆ2ª@9f1A@Ä3D{-¿î3ᱶF¿ïµ>ì¤Ù?ïÿë""i·¿Éçã(®ÊÙ¿Ár$	ʄ¿» !6ö%AGNbll3FGL J1417.8+25401E 1415.6+2557?ïúiïçXH?DÞ3$û?FX@bžà?DÞ3$'?ïúëÎ8ß4?ZûÒªäJ?DPǃ--?ZûÒªäJ?ïÝ©)2´?s€…š§ñø?q+k@f¥—?s€…š§ñø?ï£0£?{ôJG2K?‡3×9y\¯?{ôJG2K4FGL J1418.4-0233¿åã­Pí]@JÓÙý6÷äÀ8>Ùtzü À;Q‹Ï¬{@Ë¿º?ú<¯c/zA?¤Ê"0'o?´€$þg#¦@Äpë$¦¨@ÓAaRü?ç¾¹ä"¿Ý=ëì:¿×_nû`^¿Ðqal+¢E¿ßÀÒÆӿáO	ß3ØAGNbll3FGL J1418.4-0233NVSS J141826-023336?ïþ|SäÐ?!L›P7ü?(:Á²þ¤á?!L›P8 ?ïñÙז¦?kt"‰Ø?\MÐPÒµD?kt"‰Ø|?ïÍÏ(;ƒ?«CüS±?ykõb>À?«CüS³?ïÏ4y2¨b?`';ZÙQˆ?xeÃf«Î?`';ZÙQ‡4FGL J1418.4+3543?í¶öÏB¾@QfY_í¦aÀ8'cxu\£À;À®ã­¹â@á¨0¶+@ Á['—?Ÿ¸ådHT?°ídášÓð@ÙÂ~•1@fTȯ1?Ô"g^¿àEí οâøòÔô¹¿àŸ¼ÞÃp¿ã¿''Œ6¿é¨¸á2ŠlAGNBCU3FGL J1418.5+354387GB 141615.9+355650?ïýÃTw;?)*…Žµ¸?1å_¼F%/?)*…Ž¶)?ïö–ÎZÄÒ?k{…ª8I?RÒcJv]ë?k{…ª8J?ïÜØü:?zW±!~'S?q÷"¿cq?zW±!~'_?ïÿã$KÅ>á¤U8±ý'>ìÛñ´9aÅ>á¤U8±øq4FGL J1418.7-3504¿Ûwô®*ÕK@8xW£UÀ9õ\ŠD'À<+!xö‹ã@qªqX1ð@.…Nˆú?Ã;™‰(ˆ4?Ëz$‰LD@Iæ?@0kؖ/?ãaýKÙÆ¿æšáBO°Â¿ê]3ímVE¿êšn«¯EÓ¿ï VíLŸ¿ï÷6ÍòfºAGNfsrqPKS 1415-349?ïk<­K?•ô«zÇh?'ŸØj_v?•ô«zÇh?ï˜×R¥-?¡$ðÙêƒý?‰Ê+V¾´q?¡$ðÙêƒý?í¡"½Ö""?£5¯ÓÒy?²óbKc^?£5¯ÓÒx?îCKxº·?"eŽÈ'Q?«ËHtTx?"eŽÈ'Q4FGL J1418.9+7731¿æ˜ŠLúu@CI›Oe™À:^§Å¬GÀ<u¹&&Û6@ fhê¥%?÷ªˆºNE?½ÊèF$ý?Én#Ê	£î@aNÏq@Ñãá'Tý?î!ƒ†Üþ¿Ô?Íà?dÅù1§¿Ì%œq».¿à:aÙ¿àÅþ¢ûrAGNbll3FGL J1418.9+77311RXS J141901.8+773229?ï@G5§?˜Ñõn×ʚ?—ýW\ë)?˜Ñõn×ʛ?ïîŸ[sÛ?sg¢±
?a`¤Œí&&?sg¢±	?íëræ—÷M?£)«Š¹E?°¤hË@E?£)«Š¹D?ï&ÛVÐ'b?&Cùx8•?›$•%ûí?&Cùx8"4FGL J1419.3+0444¿Öa|$­@M«=ÈK^À:¹Ïþ°t§À<†ËÈ1]@ ‹ÆGLš¸?ûÑÁ(SÜ?Ñi‹ T?Âxš$W"?ôÈoU"qD?öh\૦â¿ïû9\B 6?ûª0¿ãA؉B	¿×­eL`¿²lTg
{.¿ïü-þ@`AGNbll3FGL J1419.5+04492MASS J14192748+0445138?ïúøðþ%»?G!ú€®|±?D<i‡?G!ú€®|Œ?ï㻯ô9>?‰ÓŽÉæ?lDPÆÀc?‰ÓŽÉæ?︨Al§Í? "?d¡?Õï¤Ö? "?dœ?î_©@QJÀ?šÖ¿É»jº?ªkúëT!?šÖ¿É»jº4FGL J1419.4-0838¿é_Þ§váš@H-¬îàóËÀ8o‰u_'®À;§™Ûøó@7ë@Iݙ£«?¢XšËÈÀÏ?´':,v«ƒ@?-É@ÒûO—¿ÑµPx…x¿áOY"J¿â¥j­¥j¿äš÷g«
¿æק¼r¶¿ë‡4<G®ëAGNfsrq3FGL J1419.5-0836NVSS J141922-083830?ïý)ÿGg?0m°P¼©?6°EÄÉj?0m°P¼'?ï÷ZÞÁìG?cáÞøù…Ø?QJB|'rh?cáÞøù…Ö?ïÏtŽ_Ì°?;Úw-¡?xE¸Ð§Ü?;Úw-œ?ïþ®IÃC´?íЫ›fö?%cËÄ·2?íЫ›g¬4FGL J1419.5+3821?çÇï
™÷@QfÙ×À9×À¥wnÀ<=®ä"yw@ùÁ3£'@"ª¼×ŒC?·‰êá¦?ªA… ,I¤?ð\Kv @
ÓìÆè1W?ê<C²\´¿Üœ?¼-˜?¿çßáa¯G¿çç×_w߶¿ç9ö X:)¿âzŠ&_AGNfsrq3FGL J1419.8+3819B3 1417+385?ïø?¾1ð?DùA[ZØj?O;è;2?DùA[ZØ?ïü–••FÈ?R?Ð}õôM?;KSUÉÅ?R?Ð}õôL?ïÂM4v¶?|–âÛ©ÍÇ?~ÙeòD£ç?|–âÛ©ÍÂ?ïãèíÂP?Zó
Ͼ'}?lä=®l?Zó
Ͼ'y4FGL J1419.6-5153¿æmڒ›@!Iz»ˆÀ9W"Iô?ØÀ;¨e­ÙÂ@	$ÕøD @§£Àd¾?·<TÄþLL?´4ƒjX8{?öƨü
,8?ô¢=õƒû"?ÉZB×%+¿âŒ*°­²U¿æ;Þ}yR¿æ~T>p©
¿ç,åÁX¨¿ðAGNbcu3FGL J1419.1-5156PMN J1419-5155?ïsÂ[¨»?ä+eª$?'‡´ŠèÕ?ä+eª$?àûœP3$?ԇp.Ûít?ÞÇ_™·÷?ԇp.Ûít?í®íNVJœ?¡/r‰½Š?²ˆ•M«)?¡/r‰½Š?Û£yDŒé]?·
í9Þ)?â.C]¹‹Q?·
í9Þ)4FGL J1419.8+5423¿ã¦Ë[Û0|@M&É[ÿWÀ8íL§xnÀ<MäHêT@v"Ž¾@¿–Aö?¢K†¢W>'? –:iˆYÖ?ù×Ì%Ýà@F˜T _¿µ
[b ¿ãÔ ©Óy¿å4°
õ'¿äØuâÛ,¿è!gßjr¿å¿eÁ$øÞAGNbll3FGL J1419.9+5425OQ 530?ïûu¥iÊ]??ûË÷÷Æ¥?B)jX֌º??ûË÷÷Æ«?ïû'šµm?U³5"ŸÍ¨?A¹•+ŽM'?U³5"ŸÍ¨?ïÞ/jsnà?t×*Ëâþ?pèJÆHº?t×*Ëâþ?ïÿL.®Ñ?
}	mf?z'ª&
?
}	mì4FGL J1420.3+0612?íÉÛ<'£µ@N!	á*QãÀ:š¢Ûa»À<^{Ñ1¶[@9÷8Ü"@®"ø?¼'¡Æ3+¿²Ê'+'u?õ7u'c/@ñ.ÖØ?ïô˜ú7¿à×Nó[¿ëâËf›@¿Þ[*4ï ¿ã«ØáX&¿Ýº¹9r•AGNbllSDSS J142013.69+061428.6?ïü(ÛP7?6?ç	¥//?;†¹%~PÇ?6?ç	¥/2?ïû¤ëÐ)??SÈÈë7Kä?AlP¿[?SÈÈë7KÙ?ïÞw·äÛ»?pF?ô·Í´?pÄ$
'"g?pF?ô·Í³?ïኖ¡±?\懃Èã'?nui^Nâ?\懃ÈãŽ4FGL J1420.9-7920?èûT%ãÀ186†¥À9ÍCÿ3QfÀ<Ќtíé@	6rWá=@±›îÞp?¾Ï8
û?ºRýRü|=?ýs՟Ú%{@Ñ
è èÃ?﫲~lí?ÈJw]¼"¿æ8ÿûÎB¿æÖT5{¿éˆݬ!¿ïûVƒšTAGNbcu3FGL J1421.8-7920PMN J1421-7920?ïlÁFyb? œmõ'¢?Rg×0ÓÙ? œmõ'¢?ïW}†Ýi?­†å¤ã±l?O$RÆ?­†å¤ã±l?í«çN¿"å?¤¨nüØd?² ÅŠØÒ?¤¨nüØd?í"¬DÊù?ž'h¥X¿?¶êÙ¨7›?ž'h¥X¿4FGL J1421.1-4614¿ÅßÅ<Hn@+¹¼ýKð™À9ü]¦¤DÀ<
rÎ\@®ú²Ž22@ÑÕùµ?º´Fn#t?É	ËÛ¶µ@Aü#Òm@^06Ô}¿à'$,Û¿ÔiËá'n¿ãÕ2ÌÛæ¿ç›xqοïX(ñÿŒ¿ïÿ*¸:n'AGNbcu3FGL J1420.9-4615SUMSS J142047-461431?áó‡élN?Èv]~Í¿?Üð-'ée?Èv]~Í¿?ëê´ý¤®í?ÃuÍRüÂM?ÀU,	mDF?ÃuÍRüÂM?æëºr?·ãz"Ge?Óýò(‹Ï?·ãz"Ge?ëgrªu¼ð?¥5ð0ûfœ?Âb5V)=?¥5ð0ûf4FGL J1421.1-1120¿çrî@Fæä:§›»À9ç"UUÀ<>¨È
Æ-@"/¥	9@;û"?¼a؍bÇ?À	WC¡ë@ÿ|í'hs@
¡©7ò4»?ãS¤¢Œ1|¿Þ*߈'4¿äåZ—ü
¨¿äH!ÂG³¿è¾ó…ô¡¿ïêñ°±äAGNbcu3FGL J1421.0-1122PMN J1420-1118?ï½jîìëè?|!"'?€¥DDż?|!"'?ïù¼è"R?YtLîÌ?I]Ê?YtLîÆ?ï¨B¯Œã?ƒy0Fg'A?…ïT Ç??ƒy0Fg'A?ï{A=kԚ?v ×\NFÔ?—ØR…lÐ?v ×\NFÚ4FGL J1421.1+3859¿ÕCٌiÃ@P÷27Š°ÉÀ;‹õl(GÀ<_±´B'L@Smfò'?ð´V´A¼?àœBUåå£?ïü{±QFD?øÞÅ7­w@	(ïÀAÏ?ì[Åޜ*¿î·¾b¦¾E¿ÅZè	ã¿êÎ`ÐU¿ïð&¾°ªW¿ïýÚ rfOAGNfsrqTXS 1419+391?ïù£ïИ?Pgoc…ÁZ?Ip@½ŸŸ?Pgoc…ÁQ?ïúü[Ï?fë¶'\ö?D"ˆÃ ¹?fë¶'\ô?îIš"ýñ?šÑ"WV0L?«fVÀ ï?šÑ"WV0K?ïßÖîE?i€r'?pýÝ1â?i€r"4FGL J1421.6-4819¿çÀjŸjٔ@'Àì1"À:…ñ7`ÆÀ;öp5ó@A- Í›@fQó蚉?Õ½1ø?⑀üâ5@	«f/ßÁœ@‹\¿ô?ï«ÝhüBܿ݉EcŒl_¿êˆÂÔ&¿é²3ž½ð¼¿ïÿøsCÄ{¿ÓÝ¥q"AGNbcuPMN J1421-4820?î¹Ïµ?²°'Ë—~?¤c΄É?²°'Ë—~?ØèC*ôı?ѸbɇH?ã‹Þj…¦?ѸbɇI?è'E"ƒð…?±™@ÀĆ?ͺéíð=ë?±™@ÀĆ?ÔêUfNjÛ?·\㑠àò?åŠÕLØʒ?·\㑠àò4FGL J1422.3+3223¿ïýCŸ6i±@Qh~AN~éÀ9t‡Ù}µ8À<n±lôõá@zæ'Ì@ù©™èt?©úg\'¹?§‰ÎÒ`‹?ùzà…v@·½WÓ|?ïÿù³>†¿ã€!ùO¿æXÞW(Ü¿èwhð?ï¿Úgéek•¿èg˜_ݶ)AGNfsrq3FGL J1422.4+3227OQ 334?ïÿ}w÷£­?ý¹¯(à?QŠwÓ?ý¹¯(æ?ïü¨åÎIû?OÇ͚;j?:¸Ñ°+ƒ?OÇ͚;c?ïÚ	L¢C¦?vÉç¹ Œ?rûY®Þ-d?vÉç¹ Ž?ïÿöÀgkÝ>Êí'3˸>Ò1(D‹`>Êí'3Èû4FGL J1422.6+5801?Ð÷«æàÑ@K›<Ž%ÈÀ:ސ†Ë`¼À<˜Wk àJ@ Ü}78P~?ö$‰íT+Ñ?ÄÂ'ϨŸ?γõ:,Ü@
›Háa«@I×áRëµ?ÓT^¦ÿ^¿ï'ᐩ0?åôB'KÇ¿¬‹Ü"à¿×éû[Ök¿Þ²'#ƒ'ÇAGNbll3FGL J1422.8+58011ES 1421+582?ïfú%Œu¨?‹ 98?" »NqK?‹ 98?ïðñà«8×?qºq͉Ž?^>©ŽT?qºq͉'?î<•=@ï?ž­ÿp÷ºg?¬6¬+ÿñ?ž­ÿp÷ºg?îù0'ˆ4L?1äÝm? l÷×|»[?1äÝm4FGL J1422.6+8150?îÂGVGi@AL\1Y>À;¹$Øý\¸À=\-þ@@©¤æ©Â²?õ'
0Ûj?á4ڂ˜?è•Ú\ØH+@»7^;º?ðuR½g¿ïÿb`ÈAÎ?ïÿ|Ìy?'ëËRÔ¿àÏ8·×rB¿èqgù
¿ïÿþBe«+AGNbcuWN B1426.4+8205?ïÁðÎ[.ª?¬ÉQ^VEk?˜Òh«g?¬ÉQ^VEk?ê2¸ì"Öƒ?Ïò,gæR?Ç5M°¥ð?Ïò,gæR?íkDº?¢»P'O?´§mÚ/™?¢»P'N?ÚùXöIàZ?»'²mHþÖ?âƒS"ÛÓ?»'²mHþÖ4FGL J1423.1+3738¿Íù2dän@Q#_€™À:îؐOÀ<JãÁÛØ@ýÔö¼à?þ׶»%?·«u#I?€¸!Df@	ŠC»@Ò÷BOù?àã;z)'¿Ûþ\;ë¿ÞÀgmÍ¿ÝR•äƒLÑ¿é_6&,ºs¿áš3½œ®!AGNbll1FGL J1422.7+3743NVSS J142304+373729?ïï‡6¬½ý?]\sR²?`xÉSBÌ?]\sR»?ïú˜¾>–´?YÍϦ-À=?E¥2Ô?YÍϦ-ÀB?îò!Iz©?—œ4,§X? ÝëhUnh?—œ4,§\?ïÿ$Êaxö?
²8ŸMúE?f³Ðá8?
²8ŸMúy4FGL J1423.5+4524¿ä;Ub»¶'@P'û?¦ßÀ;>eV›îÀ<å'ê)Ôæ@§$íË#@‡±¥)Õ?Äßʇù¿–$ƒºVŸì?Óâ:\È-@K>ôŒÚ?ïÍ8ÝŠ¿ãà'ód¿æ	ˆt®'Æ¿ÙóÿÁ–¹¿ç-ß×kŒ@¿Ódƒ7W…"AGNbcu87GB 142138.0+453705?ïû;·%"?<ÐÉXt¿?C‰#iõ'?<ÐÉXt²?ïüd_ºöN?SUëÃ^ø?<Ý(M•»?SUëÃ^û?ïñÈó$¨?n ²¦¥ïÿ?\Þn¶°:?n ²¦¥ð?ï磪´ÁÖ?S@o@ûz…?h\UK>)!?S@o@ûzˆ4FGL J1423.5-7829?îÁûçM&À0x,äd™À:ŸSÌ/îÛÀ<,ƒ2O¥@ö€»|Bq@8xñÝ(?ÇŃ»5÷?ÓscúÑAü@	ÂsBûÅ@Úâ9E›ì?Áùß?>¬¿ä¶Ñü·v¿æ[`Fþ¿ãMf H	"¿ïÿôÕ÷?íx= ™AGNfsrq3FGL J1422.8-7828PKS 1418-782?ïÚ_à'¯[?u˜ÁüçŠ?rÐì(RM?u˜ÁüçŒ?ïáúÎùÜ?–g¯§TÖ?n1ý$?–g¯§TÕ?ëü=©6¾k?«ReR°y,?À	[%W?«ReR°y-?ïÝgžd?ehÇ°R1?quþÌ0Îc?ehÇ°R64FGL J1424.1-1750?âûWî4§ @CÜÛ7ɚéÀ:³Ú°À<ixX×1«@ œ­çYk?ý&Á½¥?ÃÙjM%Î?¶¥"Ÿù@Y?ô™6Òúä7@
ŒŒ÷¿ïÿ;ÒDÜ?ïüé)ú¥M¿ÛßÚ¾[¿ÞÄÑ ñý‰¿ØI3$Ň3¿á>—jjAGNbll3FGL J1424.3-1753NVSS J142412-175010?ïÿ‰g3¥ä?Êf`US?
¦3†…?Êf`U–?ïýx€N	?K§²Ý$?4?{ýÂÌ?K§²Ý(?ïôXÇ=@œ?fàïÃp#?WNq…~É´?fàïÃp"ð?ïûlšq"m?3ýS½ØŠ	?BM–9îNJ?3ýS½ØŠ4FGL J1424.1+2917?ìË9s›s9@Q`ô^NÀ;ólàÓêÎÀ=|ñÃ&[@!mÇÏâÖÏ?úA×:äØ\?Óò۟x€Å?¿ÿ°ÏÁí?ë)À°3å@œÑOŒÊ?仪›I¿ïûÕÎÔ
?ï+Îð"{r¿Ï<ÑW "_¿ä.Äf¿Õ
5ã盅AGNbcuNVSS J142408+291800?ïý?Ÿ6wJ?0m"±4?6LE­C?0m"±4?ïûæ¢|v:?Zº<x¤Œ"?@ev'k?Zº<x¤Œ'?ïðGzS?cð!èþ×£?_qáõ[N?cð!èþ×­?ï٧ڎOV?eçˆv*M?s,¸ØTÁ?eçˆv*M4FGL J1424.2+0433?íq€'Ší‰@M3•1ã¨À9ÚÃvõØÀ<(9oV•@Xlþ†c?ÿ®Gx?¶[²Ù0³Q?ÃLßV½&@4±?¨Œ|@­¡kõò?ïGŠ¾4ƒ•¿ØÓØDO:P¿á3§—‰!¿á'­"ãY׿æå>³™õà¿ïÿôw5ÁƒAGNbll3FGL J1424.3+0434TXS 1421+048?ïýЧÒ?2:™ø?7IzÁw0?2:š?ïù6Dƒl?i7ƌ0¼	?K&ï©òQO?i7ƌ0¼?ïkêv>ì?Œ>õÐÌåß?''¿Q8"?Œ>õÐÌåá?ïüZË`§E?(}ƈY?=)¤úÅÞ¾?(}ƈ4FGL J1424.6+1447¿Ã'ŠKém@PBçÀn¹À:iȉq-jÀ<uÑá߃‰@äk*Í^@7ÆZÂÄ5?¾G\5
"ï?"Æ4=…'È?ח-ä>ÙZ@
ô(Ü¿æ˜\þ2ËY¿äžOv_Ø®¿åÃƓͨ¿ÜTF=Ñò¦¿æÄ¢t´³¿Ý/"—Ú|¹AGNbllSDSS J142436.29+144910.5?ïþ	÷þ`û?$€Rݞ?/`€ð9û?$€RÝG?ïý7N©'?K|"@°i›?6EŒ³r?K|"@°iz?ïøéé3U?cÆa°APí?LX[¿2±Å?cÆa°APæ?ïþ{¬Nþ?W
ª†7?(E;Ó?W
ª†î4FGL J1424.8-6808¿ì§Øä¿™À]{ý§`,À8ÉBÇ$íÀ;€нV@Yà¶Bó@ç>?Ö¯¥?«ç"w³?Ì._6qV@%€Ãÿ@:Š*»À`?ïõáμ'¿ÝU|o?¿æ	àž»Âc¿é#™7t¿ç|}Ê0:Z¿ïÿ/¨;ôAGNbcu3FGL J1424.6-6807PKS 1420-679?í{{£'?¹ú*4³?´$"ãóo'?¹ú*4³?î7—˜G8?¼WPR]—?¬‡†{Œp?¼WPR]—?çéen"pÞ?´¥*l-¹?Ð-5"÷D?´¥*l-¹?èT•m(%?±à;XED&?ί½ªK_k?±à;XED&4FGL J1425.0+3615?é°äÂÏz@Qn'"šVÀ9؏AQ(À<
v{‡`@ SEµöâ?û€ û?¶ØÐç
À³?À,2ñÅ«@YQûuVÄ@TxžÍ5'¿ìâT1?î#Cœ7̿ʸÂ~À$¿×`½,à¿à±Šâ¾w¿ßIà>¿jAGNbll3FGL J1424.9+3615FBQS J142455.5+361536?ï…òă£É?VàÚÏmú?ŽƒNß
¨?VàÚÏmû?íöæpœ­?ÁÄYyŠR?°HÌ{Bš?ÁÄYyŠR?îgHô݈?ž]ÌÚ(Áº?©Žp²''?ž]ÌÚ(Á¹?çzçõÄ,b?³ôE¹?Ñ
0w§<?³ôE¹Ž4FGL J1425.4-0119?í¤
œõZ@JÒYÀe¶=À;lœù	À<ÇÏï–ü0@!à*w¢Ï?ö¡›Lø?ف9ÜÆÑ?ߎ0Ú¾R@ŸL{ٕ2@ˆžìää?ïû°&äp¿ïÿùëñ?ïþ¹ä'¼0?li|Š.¿æm›¿8º‡¿ßõ b‹AGNbll2QZ J142526.2-011826?ïþ˜
íæ?(D¤¡>?&Q!˜?(D¤¡,?ïúlÿO?\™å¹Y75?FL²ÃºÓ?\™å¹Y7=?ï½¢Q·>?' SД?€—zk'0y?' SД?ï¿ú5œE ?r1MÉ?€r˜î¸&?r1MË4FGL J1426.1+3403?àðo&Út…@Q!灃ùÀ:Kñq…À<˜Y¸Øú@zã ùµ@ÓÅåQÿ?»æþ§:l
?¹
Ùͼ5ü?þBu
n@Jzpßf-¿ì
þ‹¶­¿Ö6j?Žá/¿âYÍ "¯Ó¿à™_æÌR¿ã/\äÝdË¿æ@U$õ'ÎAGNbll3FGL J1426.2+3402RGB J1426+340?ïû&'$Å®?A¿/Ãò_?Ce·léEÇ?A¿/ÃòH?ïúhÔ«\?]CUæΉ?F\­Rž?]CUæΏ?ï䬕5K®?tY^ç™F#?kSjÊ´SŒ?tY^ç™F/?ﮁBÊU@?oU©9Ÿ.¸?"_¯Mj¯Ú?oU©9Ÿ.¹4FGL J1426.4+3625?å[¡T¼jc@PõöM½ùÀ:Tغ@ÙÀ<F<"¸@/fRÅIÌ@A'Ã'ë?¿
SO³F"?—'(6êÎ?Öˈü@›©×Te2¿âìËð¦¿å:"yÄçü¿ép÷б^¿åË¢Ëq'ú¿á­òKâV¢¿ïÿÀéz-AGNfsrqB2 1424+36?ïúЭ&‰?F!;ÑÚ,v?G½KeÞo?F!;ÑÚ,ž?ïúIþ'?a×zՉ"N?FØ»¯ÿx?a×zՉ"Q?ïÇSQº?|o8z,ƒÛ?|VWp¢Ž?|o8z,ƒâ?ïäûèY=?^HÁl"ú­?kó¦ÃÊ?^HÁl"úª4FGL J1427.0+2348¿Ö
Â3@Q
´·,À6Ô{Ås<8À:º¿&¼@` ãzcH?ûHcF uÁ?Žec~võÍ?­ÃŒ #$â@37ÿJÎZ@Á¿}ƒä¿¼Fa
a"¿Ñ˂Iñ»š¿Úú¼#\Q¿Ø"a`î{¿ÞïҋR¯¿ÞÖ-¾ÕlAGNBLL3FGL J1427.0+2347PKS 1424+240?ïÜÒ*$±ó?¨Îº¹b.?q–êí§†?¨Îº¹b/?ïäŸ
/¿?˜åsÅÏ?k`òêÐAj?˜åsÅÎ?ï˜U¯†…?9Cü(1{?‰ê¹T^å?9Cü(1x?ï xE€aç?uºÞÞ:È?‡áîŸç†®?uºÞÞ:Ê4FGL J1427.4-1823?îã\¥O@Co`|A™þÀ:_'‰±ÅÀ<YðHÒש@ l)lŠî?ý&ÆÞOâ?Âɋ9Y'î?·õºgš?öVuÂú»ó@žé€â"‰¿Òº|þƒS1¿ì¿"zM£ø?«p=]a7±¿ävH@áqŸ¿ºÝå_&s¿è1D±	ø§AGNbcuNVSS J142726-182303?ïù«8ªÎ'?F÷†»(K?ISTž¨?F÷†»(-?ïü\ëyHÎ?R•;°æé?=¤5¹šx?R•;°æÛ?ïÛ*¾ÎŸ†?|ÖñnÓ¤¯?rj ˜°=~?|ÖñnÓ¤°?ïÒ31,MP?fïx:ïý?vægiÙXI?fïx:ïÿ4FGL J1427.6-3305?˜¢«4DÙÿ@9–r§½HËÀ8ŇB_ À;Ȓ%1ñ@B†Òeh@–'³ÌJÇ?¥C8cõ?¾"yNõ†@¡aä÷f@SÅm2¿Õ©ma­D¿Ö¹ã»üšñ¿äe0Áhë|¿ærᏥ¿ål¦â,…o¿æ\_©÷AGNbll3FGL J1427.6-3305PKS 1424-328?ïög6
Y?Q¾Ž/Ás?S0á"ëNá?Q¾Ž/Án?ï÷~UÝ%?e-²¨Wh?PáTEµÂ?e-²¨Wb?ïmѝ°×?Ž€ƒK˜þ?'EÌIÿ%3?Ž€ƒK™?ïóª[íûò?EÔâµ¹ó?X«H$à?EÔâµ¹ä4FGL J1427.7-3215?Úªã$c@:X_9K{)À:-70îµUÀ<C¯æâøˆ@¢Éübç@ѽaõ¾^?¹ô%j‰?pGڊ$±?·­=+H@å?›\'?ɛj^˜'¿èO¯'Âe¿âPmk=e¼¿âT§BÔ¿ãÌ'áE¼¿ÈÚ*~…AGNbll3FGL J1427.8-3215NVSS J142750-321515?ïý…-kˆâ?2Åh•¬¦?3֔£¹Á?2Åh•¬¥ñ?ïþÇ°›/j?>Ç,_¾m?#"öM	nõ?>Ç,_¾j?ï÷l£]"?dzˆ)w?Q&¹D÷z?dzˆ)?ïþÃ+=³ò?ïxJw+á?#ÍL$ÀÛê?ïxJw,¯4FGL J1427.9-4206?á š;KŠ@1DûC؜åÀ5µ¥BDH.À:'¨æ=·@áÃ;Ôl~@Å,?#+~?}P>à$=X?¶­ÿ7¿E@1tÿ†]}@#ÐÜÑқ¿Áã¸á2Š¿ÝÍ+—]7¿ã¢U_­å¿âÿÀ?Ѐ¿ç¡¢4¿¿ê¤0+@öjAGNFSRQ3FGL J1427.9-4206PKS 1424-41?¸7ûº?DíN²?Œò•?DíN´?éª6sZ9?ÓӇȮM?ÉW&2•¿?ÓӇȮM?îÒS0»í&?¯Axh?¢ÚÌôA-·?¯Axi?é2aW?Å;õ`ÓéÝ?ɋ7¦z£©?Å;õ`ÓéÝ4FGL J1428.1+1629?ïö³_¶œ@PMØ/×^ À:EçjÝÄÀ<UŠ"C"@ŽZ"Zî
@‡ëy`>.?½?s³VB?½ËÓþo\.?ûöÚ7›@§EaE•?îäӉp#¿æ2-¿€Þã¿å¾Tdc¿êß !s¿ê}'gv0ß¿ðAGNbcu3FGL J1427.2+1610MG1 J142813+1629?ïý†dÈ¡«?764v§t?3ÌÙºò¬û?764v§Š?ïÞ_	ü‹ß?Š–ñIµ?pÐ{º?Š–ñIµ?ïÅÙÕyú‡?~=ŸÑIç2?}C¼B?~=ŸÑIç9?Ê'?'=yk‡"?¦n"_¶ê?'=yk‡"4FGL J1428.3+5635?Ïo—¨cì8@Këæ`ɊÀ;rrä#+À<€ß×@ϔ*ÄϨ@Mv«Xÿ?Ñj;<ìðY?ÃãC]©~?ò†	êdH@Pÿߞ¶¿ë¦ %9um¿Î›C踿ålZÁ'œ¿æ£ßÙj¿ïÿb%>Ô?ètÛߏG0AGNfsrq87GB 142651.1+564919?ïûIÕxcˆ?C0ÎN"K?BتqáN?C0ÎN"M?ïü̕FS¿?Qüàõ«ò³?9›UÍb¤?Qüàõ«ò·?ïkèÏ$ߋ?‹6žò¬ž?''æds?‹6žò¬Ÿ?ïðñè
a3?Pg%s"êÍ?^/ë=Ÿ¤?Pg%s"êÈ4FGL J1428.5+4240¿àOšT!ôa@P9©¨–hÀ9t"à4êÀ;ÿO†Pº@!¥ÿƒƒX?ù°³â;ë?«6ý[ú–x?•'ßÿë™R?í?jCj¸Û@f;¥¿é1•Ùñx~?èR€f­¿Óù
'åÍû¿ÙL;l茿ÊÓ¤—Ïj¿Êß"$m¹AGNbll3FGL J1428.5+4240H 1426+428?ïü¨Ö+Ñ¥?7\*—
È?:¹N¡rçT?7\*—
à?ïûl‹À&°?YD5Pù~?BMÐÿeA'?YD5Pùw?ïæ7ց?sDÏm†>Þ?iÈ)~îq5?sDÏm†>È?ïޏqªµ?cŠ«×ے?pú8G*¥ä?cŠ«×ۋ4FGL J1428.7-1017?堄gË8@Fà:S¸ä¸À;I|­ÐˆCÀ<œFÙÙ$Ê@#
‡þZä?öõbÓ3ï?ӗ…"P??ÑI¬|]I?úèââ¸Ç\@þÁFÆ8¿ïÿT_™?ÝN=»!~«?6Ã
¬?ÜZ'±m˵¿àn¹ª?¾ëƞE·AGNbcu1RXS J142844.4-101801?ïõÚ´^?P"î ¨Ù?TKð—×DZ?P"î ¨Ù?ïûb©— H?WÙ4Ӎ?BuY£~ܗ?WÙ4ӊ?ïÄóD®…«?{¼­ki0?}†]¨½*"?{¼­ki:?ïÒjÌS"Ü?j<°¾\³?vʙÖ6v?j<°¾\µ4FGL J1428.8+7429?Áº²ñç}@D'À~áÀ;s֑q­À<ÿž)\ñ@!}@¢‡~å?þË׿o8?½Ӑ¶¿¶s"ölƒa?ú{x| @	#pš…?ïâ½—¥¤¿¨nâXFµ¿æwÂ,ém¿â°â`‡Õ¿âd ()ö?"cþ	äAGNbcuRX J1428.4+7429?ïþ?óH?$Y«›ïœ?'àː[?$Y«›ïE?ïýk'QH?IA¥Ýô?4§Cmu¼ò?IA¥Ýþ?ïæÇ=Ó·û?thcýØò?i8Â,Hë?thcýØì?ïê¼BÀ#±?WCp
¨ìÎ?eC½?ÜPJ?WCp
¨ìÑ4FGL J1428.9+5406¿Ï¾muJ7Ò@LÑM"‰aÀ:¾VCæÀ<Ÿñpv‹@ЉÒ|97@èÃm¨z?Ço<8j¦?¿ƒb¯È°?ôOÆl`{@¶¥ÇzS¿Î~¨<¿3¿êm-]0]¿âP÷†®¿ì¹›Aº_¿ÝäYüu±Þ¿ïÿ-r)HAGNfsrqS4 1427+543?ïüàÎû$?6­n§Å?8ùˆ&ßeê?6­n§¾?ïýÌój¼â?H¨½ÕßÙ²?1˜dªê€?H¨½ÕßÙ´?ïÔù?ø?vØüåñ?uƒ`zü÷?vØüåû?ï÷ÉYUÀ§??'"=1º3?PmMT~°ˆ??'"=1º;4FGL J1429.8-3058?ï͍e†q¯@;Voç¨mÀ;&Ìÿ!³¯À<'ütðm@ ´1ð'ú™?ÿ¬ÇÔ?ˆ?ÌZ.õ‹ÝÄ?ªŸFàAÒ;?äþraFl?þ(V†?u?ï]}>o&~?ìl]¡Eà_¿èç£è§ô¦¿ØUÃ`½Z¿ì¦€‡ÏÃ?ßOµIùHVAGNbcuNVSS J142940-310013?ïôgLêË?\P#(šm?W1f+üh)?\P#(še?ï^Ãå?±l/ŽF@?"=þçžã{?±l/ŽF@?ï%—=,<?ˆjWÄX&§?Œ6š0´ñ?ˆjWÄX&¬?îi®µF®?šÚm›=p.?©e«•‡?šÚm›=p/4FGL J1431.1-3120?ïÿ6t"@:ßlœ
"À9ÛÖ¶Zš€À</OC427@òˆQ¬y?þ̦6`^?¹"y™I?³¼f"HÕ1?ûº"ԗœ@-îdÍ	?ïÇ P ¿æçÌÍ£Œb¿ÑíÔñhŽ¿àŸß|&í¿Ý¡l å}É¿Üå6%+ÁAGNbllPKS 1428-311?ïÿ‰Ç¾Ã??éïü!â?
ŽO0™U?éïü¨?ïþO<?Cî)æm"'?.K?ß®"?Cî)æm"&?ïì¦9&Ô[?sÉÕ<Á8Y?cYÆÙ+£Þ?sÉÕ<Á8V?ïþiÍø;ƒ?o
R2C'?)c |G׀?o
R2C4FGL J1432.2+5051¿ï`Ù²ÕÉÒ@MÄ}¡ìNrÀ;Œ¡c'wÀ<ÓGºÇè@âõLÈ°ˆ@Ú6º§0[?Á³±]Z¤?Šo*%sÇ?ÈÔÁÔiy@
qŽ¯/Øá¿ëÿ˒:)Ç¿ßii:¬#_¿å÷·ÒiſݑÅÚ뛿é"±œ]™¿×œªZ±ý>AGNbcuNVSS J143217+505603?ïû}m(Ž?7Êáa	6?BšK]Ç_?7Êáa	E?ïýÌjêƒ?P}'óãÖ«?7™œ¨«ì°?P}'óãÖ©?ïÛÖ¦n…»?w>cШ1í?r¬È½!û?w>cШ1í?ïýg$«œE?&(ƒe¸Z"?4ÆÚ£Ó?&(ƒe¸ZS4FGL J1432.8+7648¿ëÏu!Dpï@Co8q`•lÀ:ôÞü*ˆÀ<Äh-ƒ@
Ž+§M·@Œð=ë?ÀA°¹ñ¨Ï¿±¸©)Y•ž?ðôu£KÜ?øS¸8ìË?Òpõ5¡¢}¿ä‡£'¦ô¿åJù"–,þ¿æ°ÔéÑÀR¿ÍÇNH7|C¿ïûܟ¨§TAGNbcuGALEXASC J143211.35+764355.6?ïâ¾²äv?g—
ҙ?mAMû‹?g—
ҙ?ïÆð%Cö?")È·Ê?|‡í^ù?")È·Ê?…`¼Ó?…œÆH	n?‹Ðž§ÐË?…œÆH	l?î̊"qH'?"5%#$ñ?£7VÈëvù?"5%#$ñ4FGL J1433.0-1801?ÊTU¤p80@CIM½øôsÀ::DZ°èÀ<~ó%&*@u2¹e¼È@(ãúü?ÂÆñÁxÛ´?Õ}BuñI@	'^VÍl/@ù
ÒÁÙ?×Ýê¬\¿Ó(ؼD>s¿éS³`À	E¿êR·ÈXÉÆ¿èÕÙ ð¥ð¿ïÿì»"AGNfsrqPKS 1430-178?ï|ùm_êû?'y€vœÌ*?`ÒT Á?'y€vœÌ(?ïû›Uìé'?XÚ	ã`Éõ?A'¨LYº|?XÚ	ã`Ê?ër¤'§:?§´iÎ'‹‹?Â5oac³?§´iÎ'‹Œ?ïõrÚÄ÷…?AÄKy—«ÿ?UJvóÝ?AÄKy—«ì4FGL J1433.7-7304¿è*1Q¢_ÆÀ'`†`ÔÀ;°¥R4€:À<Ï0é¬×@#1©kž´Œ?ڐþ?‹†1?ãќ	¶b'?ïù½€Ô{Ã@®ì?þÛ3,}6?ëå² ùõ¥¿îޜ¾H'¿ïԋÝï4?ïŒv›gÏó¿Ç{ô'žUk¿Ï¡&Á4éAGNbcu1RXS J143343.2-730433?ïÆ@19@Ú?z¿…'˜?|ßçc_".?z¿…'˜œ?ï×ykO~€?¨ë" í²È?tCJX@À9?¨ë" í²È?îþLúpcì?"ûWv–:O? 0XùÁ:?"ûWv–:M?ïÕfU
Gý?y±*ÙMæ?uLÕy\?y±*ÙMæ'4FGL J1434.2+4204?îWø—ŽË¡@PC¿rq7À:GÞ
ò}À<¡("V@éùK/ÿ@—!œ1ú?¶ÍàsØ(?‹¨Mˆì?ш¾ÀoœE@_ˆü"d¿áÀç@Áf<¿æÉì}l<i¿æS.°ís6¿ãFñ÷(Àé¿ê''ÿNTL¿ïÿÉ¿&FAGNfsrq3FGL J1434.1+4203B3 1432+422?ïû!1Ôså?@BAx³ç¨?C{8®0hÉ?@BAx³ç¬?ïüš*·nö?Uá~7*?;.ªDˆP»?Uá~73?ïá:"m±?uƒ—å-²?nÅkä'N^?uƒ—å-¤?ïçÂIŽ?X|q$Гf?h=¶qáàl?X|q$Гf4FGL J1434.7+1950¿é´.EêÜ@PR2LƒfQÀ8· ·›`À;¯–ú'è}@ْÔ-"8@)(v>K?£ß¾þQþ?ÁŒšBç±@´[זT@Â*­¨š>¿Å²@Äì-»¿ßÃp,¸Å¯¿äì|•|Ôg¿å1" Ü.¿è`½¨"¿ë‹q¾‰=AGNfsrq3FGL J1434.6+1951OQ 253?ïÀ±½À¢»?|}ðå
e?§!®¢Y?|}ðå
e?ïóK"ò×5?ia—¦+Ž%?YiºQ•!?ia—¦+Ž'?ïp©=+S?µ{×w'?'êÜ8Z•¡?µ{×w'	?ïð ÜÛ¯??O¹˜]Ö?_¾FH¡¥?O¹˜]Î4FGL J1434.8+6640?Ì1ùõ<ü@G°K±¯:À;1ñÛzºÀ<äŸê²ð@!gŠS*Ÿf?ù~N"ÈQ=?ÄMoßáÒm?½£Ž¡)A(?ù`¿'țæ@=qá¿ï'ëk¿é,%Â!ù?ïý7cCœ7¿Îëð¾ïi…¿ÞšÜDŽû0¿Ðï¯OäCâAGNbll3FGL J1434.6+66401RXS J143442.0+664031?ïþ·´§"?4ÐV¯w?/t"µ‡Ò†?4ÐV¯Q?ïüðµ€v?N‹I¿FÊç?8úSüT5?N‹I¿FÊÞ?ïñ9#LØÏ?hzž ©?]¹fNd^?hzž ±?ïÙ#…õ"½?bqÙwc£?sn=6!¢?bqÙwc¤4FGL J1435.3+7120?в
õ=ž!@E¼®§GØÀ<*¡/"À=˜w:Ê@:ë&ÿô?ÿ ´%6n?Ö¬æ0x?æH"Lx~—@~*šÞ=8@:¾÷!4¿ïÿúÁҝÇ?ð¿×V'þõ¾Þ¿á(ۋ¬q
¿ïþš9҉¥¿¡NöºKAGNbcuNVSS J143518+711818?íó ÒÛ?·>]ðH§‹?°g6ÿÉi&?·>]ðH§‹?îEéÙ±©?·ï'›"G?«¡g"dåi?·ï'›"G?è&˜j Š?´\iÏÁ?Ïe¾W}×?´\iÏÁ?èd³Ø½Ù?²mzùˆX?Îm0Ÿœ?²mzùˆY4FGL J1435.5+2021¿è̽÷+K @PRžì¿±[À:"F}'ÒÖÀ<]	ÆR_@!S«Èp?ÿ0L齞\?Ìã^ÊÙ?Ïqßy¹Õ@hÞ£Žåá@—Ò- ¿ï]ÔA5Tv?ïݤ@;¯Y¿æV>@¢Â¿ÈðšÝ;"æ¿è;`gÊ¿ðAGNbll3FGL J1435.2+2023TXS 1433+205?î{#W͍Õ?«¾ŽÝVÈ?¨Mʃ'" ?«¾ŽÝVÈ?ïRŽFÀ†æ?¬/nDé?•®7'ï#?¬/nDè?éŒÄ×æƒç?°Æyˆ fž?ÉÌì eðb?°Æyˆ fž?è»äB…?¶ªŠ9n?Ín÷ûÁê?¶ªŠ9n4FGL J1435.7+6148¿ïËÔuˤÄ@I›ÝÁç–}À;Ÿ{DDÀ<ì'ódK@ÌšY²ú@t` Ò?Ç;XE¼LÍ¿«F&CÐS.?âå7ýO@ª)¤"…?ïéóïP…T¿æxcôœ¯¿éwÙ.Úß¿·ÅC–'¹¿ã}:ÞxEâ¿ïê¶øO1–AGNbcu2MASS J14363365+6149514?ïñIµæëý?YíÖÊ?]l"2(6?YíÖÐ?ïûȵ?b¶4íÙú²?CúÝ+˜A?b¶4íÙú¯?ïºDSãÖ`?Iîª?në
g¶?Iî¨?ïíaƒþñ?UН|\p×?bžæ|
¥?UН|\pÚ4FGL J1435.9-8348¿Ûƒó]‡ŽEÀ5ˆx·¡Â]À9ñ¸'ƒ$ãÀ</R1%;ú@™]f¤S@ë=Ñææ?¼ÄŸ½Ü*I?¶ª›I?øSëõ‡:@,'y@³¤¿Ö.á_+¿æÁIÁ•?¿è½0w—¿âÎý'¿ïö6¾.®¿ïüɟpÉAGNbcuPMN J1433-8340?ïþiø¶U?'îa؈i?)`tžÚ–?'îa؈~?ïýî±¾æ?JÐý]Á??0r˒?JÐý]Á?"?ïßÈ·æ‹?r娿ô›?pð¤¹Ú?r娿ô?ïùÖrž…ü?9"RÉVÙí?H¦5…è‰?9"RÉVÚ4FGL J1436.9+2321¿—ßcqhɉ@Py©?)
»À:y|ßýÀ<Q'N"¢Â@ý1Äs7@‰
5
(?¾)j1¢ˆ?¯ç¸Ëôœ?ëSÛIgR@Ño‹þüJ¿æCŸu¦ ¿ãdc1Ù¿ä}P·
H¿é›K_ú¼t¿Ý'ù\wпïîÊM–ŒAGNfsrq3FGL J1436.8+2322PKS B1434+235?ïømË¿.—?J[µBÁ?NHÑE¢ž?J[µBÁ?ïü´®.jÄ?Q²ƒ­±e?:ZŽŒ©Þ›?Q²ƒ­±v?ïá²4¹lï?qU¢0v–?nMËF"
?qU¢0v¡?ïÚŽZ½å?c"²âa,?r÷¸Ò¡
ß?c"²âa)4FGL J1436.9+5638¿î.öFyQ–@KuâlvÀ9½Ö»cýÀ<\u¼D¿M@†òÍ<‰H?þ©GŒ†Œ?®¶cC‹	?è'u¹?ã#×?íUÙ@	äùÄQ©?íö–•[$¿äEmþ
\z¿ß1uBø";¿Ú›[慱¿Þöú2`¥\¿ÕVÄ-ÁÚAGNbll3FGL J1436.8+5639RBS 1409?ïþÄñ!{6?z|ê.²?#°íèL¥ý?z|ê/?ïüꏴ™ó?Pov¦r?8«'[0cq?Pov¦r?ïù»†¼'¬?U©2"Gf?Iå
õQ?U©2"Gf?ïôîñPD?Dÿ¡¸D?V#_ys?Dÿ¡¸E4FGL J1438.0-3128?ÂW=Ød?@:!¦'¶(FÀ:Á"‰cÀ<[¾¤ž@Ö'-ŒÚ@9ö›Ó/½?ЁôRLÔ?֖ê<Ê5Ä@våÚºÌ@	µŽª}AŸ?ﯭ7OË¿Ùùð'Íó¿ç"ré+¨¿æfS¼?¶Ï¿ïç'JïŽ4ÁRÆ!AGNfsrqPKS 1435-311?ïàm½A?p¿HH¡*?oý'B¾ü ?p¿HH¡)?ï÷…"ˆOe?dZ|zM`?Pôöïa4G?dZ|zM`?î[.
²"?š¨ôçÇâ²?ªMTÞMé?š¨ôçÇâ°?ï11»NV¿?…-Éd˜ô?™ÙȖ5(?…-Éd˜ö4FGL J1438.5-4207¿îÝ|aSµ4@0w>Õ'åÀ;g˜ûÀ<'œ£9UŒ@ ÷Öå¼]?þYÖÖ;
˜?Í0!ÌX‰?²Êö†M?äâ6kw@z7y>s?îØàkæ(¿ín¯½µƒ¿È¡šïÚîοÝÓÙ{±Ò ¿ãÉ?2Ȫ¿Ø;vBýU¬AGNbcu3FGL J1438.6-4209SUMSS J143836-420705?ïþ¾Ý'îÆ?wêÄáPO?$&á¯ú?wêÄáQ)?ï÷¢‡ÉÓ?n֙–2à?Päºðl[š?n֙–2à?ïóÜùî¦T?`ï&Çi?XF"³S¯?`ï&Çc?ï«Ä"½Ÿ?nÈ‹ÇU?…=÷P˜ ?nÈ‹Ç`4FGL J1438.6+1205?á"
r:Џ@N\UÀü´òÀ;jœ×;»˜À<Âk"ÿ@ XÙéëÁ…?ÿª¼¡Ü^:?Ðj"2¯Ö?¤PŸªª¸ü?Õî$5inY@@šÒª?ëæoÖQ°Í¿ãg¾Šêª-¿åØl¨ŸÆÚ¿ÝÊ2ÿÚ
¿âëî›S­ý¿Ë¶^Ì>1"AGNbllRX J1438.3+1204?ïû¯›rŽC?=|ôÖ¡s¥?AA'5Æô^?=|ôÖ¡sÈ?ïùÖݓ‹~?a#Ò[LB?H¤‰±Ò
?a#Ò[LC?ïö¼Ik?cy¦VIQ?Sð†ßm(?cy¦VIPú?ïÃeE'!?g' ÜJœw?~uÍ]7oH?g' ÜJœz4FGL J1438.9+3710?æγS·š@PO6&,ºÀ9+Š¿â¿À<3"l;'@λ³tâ@zŠûq%?§0¹[Uç?»¨w­áz.@q|å-ì¢@AÇn.? ©r]H81¿á¤¢š¿æNS™Û¿ä¿-½R†`¿ëö{A"ÊÓ¿ïÿþˆ0»ŠAGNfsrq3FGL J1438.7+3710B2 1436+37B?ïûŸZœ4¶?< ‰ ü£_?A'•-$?< ‰ ü£=?ïù¸m\7?[͗î·I)?IJ$Ä?[͗î·I?襤î.è?ƒxVñ,ŠÝ?†ÖÄtF?ƒxVñ,Šâ?ïüHHe…@?0Rx¶Š‰?=½¼ÓÕú?0Rx¶Š‹4FGL J1439.3+3932?î°7G;"@PêÈ`V'À9åßÁœ"À<cv­‡@ú—Ý+ê•?ÿ<ÛØÙJŠ?±ÍFšC7¸?"'¬¨{E?áªSÆP±É@¸ï&&?ï"ÞnµÀ¿àç­=»Lr¿Û×!ºdë¿áKs›Ù¿Ú|[Wð¿å§«ÅìAGNbll3FGL J1439.2+3931PG 1437+398?ïþ…Á3?'žÂïI½?.‡£ìÏ=3?'žÂïI"?ïümT­ÄŠ?T»aË«?<•Z'Û°C?T»aˤ?ïñþÁ©æ?l'Ü·à3æ?\|ü¬3)?l'Ü·à3Ø?ïç'­6³˜?UTï5Æ_ä?hØRÉLhˆ?UTï5Æ_Ù4FGL J1439.5-2525?Ë#•Ñ¯qÚ@?ZäâmHÀ;VìÔªÀ<"1í¸ÕŸ@!¡[YíÝ?ùˆ²¡)±?Ð<`CÃX?ÊH)åV±h?ü‰l«$™?÷˜ùöüv3?áÕT%B|?ït§!A™(?Ìóä餿Í=þhPK¿ÖagäjÎ*¿ã9oÀtzAGNbcuNVSS J143934-252458?ïÕû¸º$?tDä¦\GÁ?u#¢ýíÕ?tDä¦\G¿?ï¹Á㣻w?˜¨¸1{¾?‡!÷?˜¨¸1{½?ïW oˆŒ"?'52|ò?•òî{Ï?'52|ò?ìCÊ֗š?¥Ú[ò¨?¿Åá©KC.?¥Ú[ò©4FGL J1439.7+4958?ïÇÅà©]t@M–ýuâlÀ9±vi騦À<~[òoÅ@ó@7'´z@0«~žk?¯ey"øõÂ?¦&ŒÝ9¬?öa	ÐcZB@¨öæ%ä?ïôÁrüvß¿ã±b]Ã)¶¿åªbÆ[¿åÕò—Ÿï¿ÝnÊ£|ÇQ¿ïÿ–]ÏéãAGNbll3FGL J1440.1+4955GB6 J1439+4958?ïþ]o®²­?)ÀèWæ?*)Õ4?)ÀèW?ïûëi=ìÈ?UOžŸ±¥/?@R[LÚú?UOžŸ±¥?ï깄¦&Ï?f'´[Ì?eF{YÙ1É?f'´[»?ïñÓywí?JyK+-–<?\YÅ$)?JyK+-–#4FGL J1439.9-3953¿áýƒø‡	!@2_ûz_A¯À:WKtr˜¤À<Eˆt®'Æ@ ¯ÔH@ïÏÃøõ?ºB3@Êž¿ ±ÇÈªÿ?箨—›@ûÐE}8?ïþ*"y¿¼WÆåW¿éiæM§RÀ¿ÓýãÆ
–¿áWpßçÞ¿Ü -1'r"AGNbll3FGL J1440.0-39551RXS J143949.8-395524?ïû"–W91?C¡ ò/?A±¦£AC?C¡ ò/%?ïü(0áu?S…aˆ=¿Œ?>¾xôSux?S…aˆ=¿ˆ?ïî]»‹ü?gV¬ÚIΝ?ap¢DtS?gV¬ÚIΦ?ïç_ã³õ?SVeê¥ï·?h ëLS?SVeê¥ï±4FGL J1440.0-2343?îµP 7¡M@@elaR*oÀ:!…óÊg˜À<OþR€ÖT@vq·þ4@†ý»'"?¶÷*nh"g¿œ[¶ùÀ–?å®:ÀÆ.M@´t'ˆÛÜ?ïõi~sÎY¿éF
¹üæ¿á?ž¡cê¿ÙBÔ{lÝÏ¿ä¯ÄH™ÌÅ¿š"!J'–AGNbllPMN J1439-2341?ïýÑ"CkU?-‰6$í|?1víä¥W¨?-‰6$íi?ïýҗn#ì?KM# E8?1kDŽà"?KM# E8?ï÷¥fLÄ$?fHW—Ï&º?Pµ3fw¸7?fHW—Ï&Ñ?ïí¦
}:f?OôžQVN?bYò'Å™p?OôžQVP4FGL J1440.0-1530?Ĩ!%íP/@CïìÃã?À9"卍óÀ;ß>>)0{@œ%"¤DÃ@½´'l¤?µ ªDŒ¡ä?–è>€¡Ú?ä&áìÂ@@beOåñ?ïöÒYԇ¬¿ä³5è³2¿åŽF´ð75¿ãkã]²ã˜¿Ýg5c'¿åò#žj¹²AGNbll3FGL J1440.2-1538PKS 1437-153?ïügY(o?7à9Ý3©?<Å6¼ƒœ?7à9Ý3©?ïýÏ;B™?H$q%–°?1‡†%ë/‡?H$q%–°•?ïáà˜>ú?r²¬Nßz?nçgÁ£?r²¬NßzŒ?ïþɄÙ[?='ïpï‡?#g²oÊD?='ïpï;4FGL J1440.6-3846?£Û
ã3n@3S™åóíÀ9›Ò<xVSÀ;ýF[.$@!ˆjüx6?úËP`j£ã?¶>iN?S?¨H‡-[X?óÏ
D& ~@P7~òNg?ïÿîBt!¿è•Óa'¿à—«öÐ+¿Ï 	cr–¿Ö;'}E¥ü¿ÐŸ[DÊ4lAGNbll3FGL J1440.4-38451RXS J144037.4-384658?ïûk(•îB?<á|Êõû,?BS]¨FüR?<á|Êõû2?ïîô.õÇr?vLdDŠõ+?aÑ
8ù?vLdDŠõ,?ï¾AÑkÎy?€"}IƒKx?€o‹¥al?€"}IƒKw?ï'ªùŽ‡?ƒ]à8"Ï?›
 Î<;?ƒ]à8"Ï4FGL J1440.9+0609?ã;®$N@LJ@c^JÀ9¦K»À5À;ÿˆ}£–@ÆK‰Á4h@uv'[¸?¹XÙµé[y?®ê£§dˆ?ñnkÝËù@
'?úTz?í=b.$¿äõϏõ«é¿á̀v²å¿àùÊÇ9¿án"áÉ´¿ân@$ˆKAGNbll3FGL J1440.9+0610PMN J1440+0610?ïú߈NÁ²?8ráӅ?DÞÄù7]?8ráÓq?ïü•Á×?PÐ9/ŠW?;Q÷‰Gl€?PÐ9/ŠW?ïóÂ:²œ?cÐί%Aþ?X{ŠzšÆÒ?cÐί%Aè?ïÎG9©íï?cc9bŠ7?xÜc+	?cc9bŠ64FGL J1441.6-1522?äi.Uóف@CäU•:À:M0o3"'À;ßr)Zl@&+Í@ð¶ß$¾%?ÈUÛ~ÁQ?ÁªQ¢µ?øñzç&ë&@
¾Ûc9¿ës­ÁnË?ïýž%ðT'¿èš[@BH¿åªª˜Å^D¿àCnI‰¶Î¿ïÿÿÊPËAGNfsrq1FGL J1441.7-1538PMN J1441-1523?ïèòŠ'ƒÅ?køŒÈ :?g
um|9…?køŒÈ 9?ïû«iÌÉ?VÐ1Ýú™^?ASöXÌÛJ?VÐ1Ýú™]?î'j)ew? éÏlT™g?¦é]i®øŽ? éÏlT™e?ïÂnÚ}Ú?pU1]ÃD?~ȒõÁ&?pU1]ÃD4FGL J1441.7+1836?ʹ4‡)Ëà@O¢ Ç`À:€œߢ'À<}šYù@REP—@zŘûå?¿dqēm[?°:ŸŸíò?ëæ±Oí@žÍØ¯¿êéôæÇJ¿ÐõùìÀˆ¿Æ4A{†¿ä¾âÿ>9!¿àÙ O–@I¿ÛÅu€	ЎAGNbcuNVSS J144143+183706?ïø®àî?N—Òê±V?MÁD|Gƒw?N—Òê±?ïüpˆ[º?R‡ëò"6?<{¿õ"/—?R‡ëò"C?ïÎÙÕ,áQ?}¡ã—fæg?x"iWp?}¡ã—fæj?ïàÇ´V¼?Y;èÐÄ?o8ãK©BÚ?Y;èÐÍ4FGL J1442.0+4348¿±ŽÛÓ݈ù@O"úÖËSÀ:x˲À<¯Ä
†k¿@J,\\×?ÿzΝ‡dä?À"¡²í©?µ2»"?÷™WÚ²h@"(¶ØnÁ?î钀J¾¿Þƒº¿Ùõ)¿â!Êö2÷¤¿Ùk*ñER¿âPŠ\ô¿ïÿÂÞ6œAGNbll3FGL J1442.0+4348SDSS J144207.15+434836.6?ïþ|5<´z?!Ônì¥u?(<¬4¸o£?!Ôn쥋?ïûL'þ®?Tvn^Jýª?AÂÍ´I?Tvn^Jý¤?ïîÌlº´
?oŸ<–?a3"EKó?oŸ<¤?ï½b—?e¹@Âíì?€ºçZ??e¹@Âíï4FGL J1442.2+0622¿‰ão®þÛ@L>@(äüÀ:_Ê?SÒæÀ;̒Ü6¯@q§£áò@"†ŸÁÑÇ?ÆXã["‹?ÔjÛöÀf@Ž†ƒ<`@vå¿â€)«|ñ¿Ð%?•í¿è˜b'+=ñ¿æô¥žµ@¿ïÿå}ó Ì?íýݱ žÜAGNbcuSDSS J144212.23+062526.1?ï*X2ˊ?¡ît•Ê·?š¼tù¦Ž©?¡ît•Ê·?ïÐÉ3;?˜Ón]ì…Ë?wòfxâ2?˜Ón]ì…Ë?ê58UæÃ?¬Sÿâûè?ÇÏ+¨dï?¬Sÿâûè?ïu[…§Å¯?†³ '+?'TKIí?†³ '+4FGL J1442.6-4623¿Â;z‹s@(•¶^Ì>2À:Žö¨hiÀ<-_²@ sZwÅ´U?ÿȺiú?¸`u¡æv?"¾¬Åè¤f?܏Û_Œ­x@û-+û¿åՔ«W?ïúhai¿¼…
ìB3¿Þ<ǼAº5¿ã(qGпÜk:¡±SAGNbllSUMSS J144236-462302?ïø	7UÔY?K@–Öe?OÛ"¨®ž?K@–Öe?ïúSüŽ"?gÁG-ÚØ?F²
Åì§?gÁG-ÚÑ?ïì&û‰:«?iAÕ¦Õtç?cÙvÅV6?iAÕ¦ÕtÕ?ïÙsJ€?d‹Õ§B?sFZý?¾í?d‹Õ§F4FGL J1442.7+1200¿Ý>dÇí¼@MëöÂiœ|À9èóɐØ*À<1<°Švç@ €&˜ðý?úÏÀÒÆÓ?¸Äßîg§.?¼'‰¡m½7@?¹£ûk@ÜíUÔ¿ï¶PÕÛi?ìyK!K¿Û±EC_¿ÁwkFud¿âï6ÀÁ&¿Ù¤4'NùbAGNbll3FGL J1442.8+12001ES 1440+122?ïõ¶	`½?Y3®Æ­J>?T"í>䈕?Y3®Æ­J2?ïô5­ëXA?q{wÞ4dª?W"¤)O|?q{wÞ4d©?ïÎtߖ¡†?}ÇS~~NB?xŐ4¯=h?}ÇS~~ND?ïƒoÕ6W?Š•*µØ"m?ï'Y5*?Š•*µØ"l4FGL J1443.1+5201¿ê¡QFÅE@L¾Ç¸Õ¦À;X"%"À<ä@¨f»÷@È,å'?ÿ,^YQ«?Çw*Cuu£?ÀåOe´?øÄÉþ¼3"@*0aFÁÛ¿ÆǪ5¿à\¶úS¿á䠓ˆÞ`¿ß"ãÍy¿ß™Ì$0`ñ¿ç/Ç~fAGNrdg3FGL J1442.6+51563C 303?ïð1i†w?^0ý«Ì8‹?_ß,ó??^0ý«Ì8Ž?ïú;-ÿa9?[¹rv¶j?GH{Ð?[¹rv¶f?ïâ©ad_…?tÂÔ6­à?mVž› {<?tÂÔ6­á?ïmKªþÖâ?zŠvÑ·D?'VŠ %#ñ?zŠvÑ·D4FGL J1443.1+4728¿Ãä8é-'B@N&ԀuÀ:k"Úí÷ÀÀ<¡´¯Ÿ•\@r*£Í@^ïCðÙ?¾a¥'°?ÈõæA½å@37º@Ó´Ï*8¿º^-ݳÏÑ¿å¦Ï!»¼"¿ç-O>+´º¿é©ŒUä8#¿ð?ïæþ!¯AGNnlsy1B3 1441+476?ï|mï‡A?"ÉE•Em?rBwÎ?"ÉE•Em?ïX¡ºž?§á1'òH?"ý+Üè¬:?§á1'òI?íâ:¸?¢ùöOÍÿ?°èŠÆ*@?¢ùöOÍý?îuÓ¶ÃL+?˜­Ô.ü‹ú?¨¢Ä"Ë=`?˜­Ô.ü‹ø4FGL J1443.6+2515¿ëæK-ngÞ@P4t>–=ÅÀ;-ZyɺÀ<4šöå¥@#

éw¨X?û½{Uá³å?Òð'ÿ¤:‡?­•9•T?ð'ß»¼Ú@­pՀ$©¿îÖëÔÏЍ¿ïþ(ßó>?ïû»'w"?Újµ ¶Cs¿Ö£D\¿àŽ¿`}™3AGNbllNVSS J144334+251559?ïÿG^žÐ?s¸1WÀœ?Ô,&º?s¸1W¿Ì?ïû\Ü:=ü?h""¯M?BŒ
3?h""¯P?ïíö' Ì?q<'¶{L?b	}å_4I?q<'¶{R?ïø¾œ¨
?EÝ'I3H?M¥_Îh?EÝ'I3>4FGL J1443.7-0954¿év¢'@FlvJßøÀ:ÜdöúÀÀ<hô'
´@™Úk›…@\}ÿà?ÉzúÁ»!?p:ÙâãN>?¦¹ÉdãY?þÚÛô#`?¦É{ßto>¿éžÒ¾~Up¿â\~¸+¿àw@Ý?â¿Ö6h½ÕG¿ïúua«ì'AGNbcuPMN J1443-0953?ïôŽcZ
?P€F'Ÿ[ ?VãÍ9KêÎ?P€F'Ÿ[£?ïýZf˜xq?Peü°L˜?5,Ë<<zç?Peü°Lª?ïß³"(g¹?q²œµv³6?p&=ëÌ#?q²œµv³-?ïÝd¨ìµ?_Þª¢Ë©ç?qM«‰ð&=?_Þª¢Ë©ò4FGL J1443.9-3908?Ýé3¨€£@2µ÷øʁ™À7ë府mÀ;8˜Ä@\a¾¶ß?ûÃ/zA¾?œ¼åN"ø¨?¬ÇïBmÍ@ˆ®`Ðû0@ í6ϟæ?ïýÖ.u^¿¸ù§÷*ni¿Ûà«;'¿Õ'€áü}¿á8 m]Ñl¿ÓÜ.ÿò¾úAGNbll3FGL J1444.0-3907PKS 1440-389?ïù0"h?N¼ø×?K=®_ˆ?N¼ø×?ï%»ñ·Ñ"?®¸ÿ.éä?›HÉÏ\?®¸ÿ.éã?ï"ñÚε?*3Ö»®'?ŽÃ‰LRº$?*3Ö»®'?ìÛÞÚQ\î?áAÿ·7
?¹!	-u?áAÿ·7	4FGL J1443.9+2501¿ïÿ¸ïw@P,†hÍÀ7Ðe…•Ö–À;]ˆ{¯¤@ûV$#öª?ÿwÃ Ô ~?—	"ŸG¿˜?¹®œ`w	@!ìæŠ
5@ù$ƒmj¿½¼O?òøõ¿Øó¤·Yô¿ál¹–m•¿á¢9ìN¿æµ6]ŠÒ¿ç_û¹IbAGNfsrq3FGL J1443.9+2502PKS 1441+25?ïò™lÛ/ª?Uw™ØGÒÿ?ZÍ&I ­Œ?Uw™ØGÓ?ïä
$''î?ƒÛšP
4p?kõÛnm"?ƒÛšP
4o?ïQ´Ô_?"[)àH´m?•ÉelTÒ?"[)àH´m?ïýШ8?2M9C—_^?7ñz¾?u‰?2M9C—_j4FGL J1445.0-0326¿ëßҋ0,	@Hw @|ÇÒÀ9‡9+
ËÀ;î¬yp@ å"aÎüþ?ù¶ï¶àë?·sJ$'YÚ?»¼LÞRD@Ôƾ•Òe@"N÷3þŠ?ÐÉ@üžý¿æÛ§r$¿ÐúAd¤Dm¿Ðí»Ú·5¿ÒK1­>½¿äv‡EÙþäAGNbll3FGL J1445.0-0328RBS 1424?ïÚdÓõ̊?k㺫>ƒ?r͖ºä?k㺫>Âq?ïï2Ò|"?qÎk^5&t?`Í-éƒm?qÎk^5&r?îøûT9ñ{?"Ñ©k5F? pJ¼`èS?"Ñ©k5E?î]`qŽ*–?áF–íל?ª)øçVŸ?áF–íל4FGL J1445.2-1954¿ïž½ÜŠµ@A¾ýq?À;yåŸ+ªÀ<r`±¿Ÿ@öé·>E5@AƎÅ*A?Á&Ž_(Új¿¶û`‰ÆÕ?öRXâð$Á@Û³'ÎÒ?Ú'Ý¿ŽJÜ¿æCx$Õ¿µ7ýu×s¿ë)xŸN¿é*ƒ–øÕi?ÁóTöÒYÕAGNbcuNVSS J144511-195853?ïôöŒêj?RœÊÛ
êÃ?Væ+é+á?RœÊÛ
ê»?ïûÎÚCð?dn>·;(â?@Æ–ðE»?dn>·;(ß?ï›W¾¨£|?ˆ½}u øS?‰*U× ê?ˆ½}u øV?ïÝ<–Øû¾?_0Mäæ{ð?qa´"' þ?_0Mäæ{õ4FGL J1445.9-1626?ì#ÎÚx;h@C(˜ëÀ9ìã.qÀ<õHG@°jœ€ÿš@•öâJ"?·`oA{P¿¡$`©ÛS?äg]Ж@Õ@–ÉÁ¿»ƒk.ø¿é–ãô5ǿ䟗_'œ}¿ä dŽõÑ©¿ì¨þoH?½¤òé.–AGNbll3FGL J1446.1-1628PKS B1443-162?ïòüd¡~?Xl…øqê?Z6ü½¢?Xl…øqì?ïþ1ƒžs²?C±'X'<?,çÆÄÝM?C±'X'<?ïÉ^lþ?1TcI%?{pPɀó?1TcI&?ïùšZýX?<&1ÛÚj?Kі"
 Ž?<&1ÛÚË4FGL J1446.0-3039¿íjå6ýÜ4@:
§;BÌ-À:ó"PXÞÀ<nsGyB@õq´ùŠ@趽–Îä?ЯûIaô?Òcˆ»zêØ?ü|MÃØ1…@"Ì€KÀ¿ï‡Š¾4ƒ•?ï¼ë
)´.¿Ù©`J{¿èÕ@8Õ3¤¿ì%ƺd¿Ó/K²…ùªAGNbcuPMN J1445-3036?ïߑå—eÔ?r/†e½ñ}?p7
4MQ?r/†e½ñ{?ïýä?Iˆ¬bg?30ߟÙ?Iˆ¬bn?írd«êK? rŠošê?´lÚ ¯¦? rŠošë?ïêaàuÃ?Wxú¾²C?ežbŠ<ç?Wxú¾²>4FGL J1446.3+3111?×5Ç~Y@P)ú—á2µÀ:¨ñ-Õ%aÀ<©Êbh@rÝ4y@Sw[0?À&ágc'?'ùXyœVÁ?ÑÞ¸ù6@û0ÍÓ2¿Ö¾ÔãÄ¿ßâ¼Bô/¿æ"º!N"G¿ì¦á€¸ø¿»ãÆÃö¡¿ïô½±¦×AGNbcuMG2 J144640+3110?ïþöScI?žŒ£[ H? šÉËg.?žŒ£[ M?ïý¹Vÿ~"?Fe¦'<y?25Hì'?Fe¦'<…?ïޑbþž?tAdH?p·N€ð0Ž?tAdR?ïÿátÉ´>åX‡"ët>î‹<vKye>åX‡"í‰4FGL J1446.7+1719?ïÖ'äÄ@NÓ³áC|WÀ:²ìzçý«À<s›x¦@Lȯ0ړ@äÖä}Ãz?Ä#-¡?¹zþuÍs?ðítw¡!M@–më?ïá\Üyèú¿àH8³¥´Z¿ì4á=òÿ¼¿×—ÿ»Œ‰¿ë{Háa«¿ðAGNfsrqS3 1444+17?ïþcQ/èW?)r§ÆR?)Êíz¥P?)r§Æi?ïüÎ}üR?Q¬:ß*ž?9üvœ?Q¬:ß* ?ïÎ!H?zPÈ4%l?xï|ÿt\;?zPÈ4%f?ïõì,Ñ+?DšzÆÃ+?T'¦]©ÛJ?DšzÆÃ.4FGL J1446.8-1830¿¸"™Nðg,@B;½‹ç)À;·ª%ÙÀ<†šÜ¸o@ N'?ØÞ?þsŠ ÒH?Óû–
óފ?°-ÜP§?Üٗ ¢‰@—ñ¥]¿è=.ߑu‰¿å©ÊiE=ø¿é¨@[9âz¿¹B	岿ҤvÂT"í¿ïú Ë®AGNbcu3FGL J1446.8-1831NVSS J144644-182922?ïþ~š¿–u?'=´pN?(T˜¯?'=´p\?ïþbÍ=2?E©&Rf?)ß,,ß=?E©&Rf?ï쾟â»Û?f`«œX?cA`D%×?f`«œB?ïùKbGì?>Ì¿.ÂùÇ?JÒvàO"w?>Ì¿.Âù4FGL J1447.0-2657?ëûÉý\ä@=09-Œ*À;‹;26À<—)2ÿ0Í@ °›yB·
?þ³&Ó©_à?Ç£ue‡Ä/?ªugáÏ×?âNæíàBË?þ³a'È?è%¼£n/¿ïÿÿ)@k*?ïÿøsCÄ{¿è©ý·{W¿Ù,ëñUB¿±Ó	&ð.ÒAGNbcuNVSS J144657-265713?ïûñb$™?8y~¿ÿ_?@:woõ¡1?8y~¿ÿƒ?ïüjG&F?Xß椎À??­ÆÍÑ?Xß椎Ê?ï߁1üK	?pØÏU(~5?p?gÚ{?pØÏU(~/?諸‰@-?{"‹5²èÍ?…Q{¯ô ?{"‹5²èÉ4FGL J1448.0+3608¿ë5,a/¥ß@OÛKƧïžÀ8é™ÛøóÀ;¸˜SH|q@g.†?ù˜Â¤TÞ?ªF-ƒ=Y?¼üë"£C@¸á]}Š@	¸¯&Ëî¿ïb²|¿n??ïþk«IÅF¿Ñ)õœÏ®ÿ¿ÚGž¿Üí:*ž9<¿à®!`¢ØAGNbll3FGL J1448.0+3608RBS 1432?ïƼ¢G²…?¢'±'È>?|¡®Ü&½?¢'±'È=?ï>2ë´H(?¸<,Sš0?˜9¢‰vû)?¸<,Sš1?îâT |¿a?™i$ÉuHË?¡Úµø4	Þ?™i$ÉuHÊ?긱ßðD¹?®‡þÏÐ?Å8€>í?®‡þÏÏ4FGL J1449.5+2746¿íŸTª^\]@OìÏÃøÀ;ÐÄv¼õ¿À<øV6mzW@"ox.åƙ?ô•|3WEa?Ø\Kz§»ñ?Ù]لÁg@¶ÄŸä@µréµ?¾¤çÀîó¿ÝI¼ÈÊ?ïýÐÈÚп¥´£5NÁY¿ÒT9]nÆ¿ÛîH}GS|AGNrdgB2 1447+27?ïÓãTÙ?r‰Ì+}"A?v|ŽU"€?r‰Ì+}"B?ïùȲ†ßæ?^Wݘ=
?HÝ5ä€hº?^Wݘ=?ïosmq?ŒÙüS¡Ê?''\ÝQÈ?ŒÙüS¡Ê?ï'Õ>š)?¬€M׌Š?‹Š°Yxõí?¬€M׌‹4FGL J1449.6-2137¿ï²HflH@@¼Èÿ¸²dÀ:»I»4ôÔÀ<Kžã…uö@çk´"@eäEVJ?Â-`‹[¿«9s'óS¹?ê†nCªz@Òùæ‹dο×ÈçDÈ1¿âìÊ-¶°¿ìÉv7]d?±å/D;CM¿çRw@Ý@¿ïÿ‰XAGNfsrqPKS B1446-214?ïý°}ÀÛð?1pÑUå´?2|ù }&?1pÑUå´?ïý'Ñ ÷?Jk"ªÒ¬Ë?3sñrøJ±?Jk"ªÒ¬À?ïޑ_xÑ?sZbÞ·?p·|ÐC—÷?sZbÞÃ?ïþ8"µþ?!ú€ÊlÇA?,vį ?!ú€Êlƅ4FGL J1449.7-0910?ï+Rß~@EÞB||RaÀ;)!°:À<‡àmòL@ >1´Øå4?þ‡S–€	¦?֝ţ7Ó?»Ž-TÌàï?êð äÑü?ìæ¹ÏçV¿ì§'Z¸³:?ïþ¡€Ã´Ë¿êéˆÅ5ÿ–?³=ïϱ-µ¿ÝÐ$p!Ñ¿ïÿÏ=ÀTïAGNagn1RXS J144942.2-091018?ïÿíÿÄø?(z»Ö Ô?"@`÷4?(z»Ö ž?î÷K‰¿¨?¯Ë0ܕÉ? ‹GdÕj?¯Ë0ܕË?ï§øÅ´åQ?"ÈV¸7ãþ?†Βƫ‹?"ÈV¸7ãû?ìÊ×sB?§™ø—u?¹¯ùDgÍç?§™ø—u4FGL J1450.4+0910?îçÚºhëÚ@LT°ò{²ÿÀ:7s	â×ÑÀ<e …F%~@´—Â;ú@æ3
9?Ã
'åÍúŸ?ÅëX¦4]@&¤û¨'@SF¶È©}?ì!åbÅÇö¿Ù8¸ãá¼H¿åÍà¿åq•n'¿é{NP¿ïìŽ:AGNfsrq3FGL J1450.4+0911TXS 1448+093?ïޞüßá?k—à¬Îu³?p°ðv?k—à¬Îu´?ïüW&"œâ?U¿h?=FÎëòZ?U¿h‰?ïQ7îü?'FZøÿE?ÿ5Ù Ž?'FZøÿG?ïõn'½B?B*‡Xe"?U#Ü܅{e?B*‡Xe4FGL J1450.8+5201?ÖùdŠ¬"@LEåóöÀ9¯UªLoÀ<P)µ/ë@7Ž`U€:@ ÷üü??¶2¬`×ÂZ?¼ŒÛ›Ï¿@5 üÏÊ@£þ·Öp?í/B]r¡Þ?ÖؽÜD"¿ã&??#€¿á*™Á²'d¿áÚŸ‹Ëü¿ïÿú÷''ýAGNbll3FGL J1450.9+5200SDSS J145059.99+520111.7?ï­Ô_Wªñ?'ŽµS*úï?"Šè*Cò?'ŽµS*úï?îŽ>0{âê?¹›³öu½?§øAÑ\?¹›³öu½?î®]Ùx7?™E'áúNÎ?¥"h~܃?™E'áúNÌ?ç×
'b0?²WÁqHb<?ÐQÁêû;¡?²WÁqHb<4FGL J1451.4+6355¿ïÚÄSӉ@H:A€ÓÏöÀ:ƒŠc›±À<¦p‰Õ×8@ "6}•'?ýNQÒÓw?µxõµ#bÜ¿€ÂZï
®?Ì©3€
&u@à±F?ækҁA³ÿ¿áŒ&ÿÉ#u¿ß S<h5¿âˆéH-–;¿Å€¢è!çܿʹÁáAGNbll3FGL J1451.2+6355RX J1451.4+6354?ïþ⋰i?El&ú€?!×Döùx}?El&úŒ?ïþæV­$?FKu´¤x?/š•-ºƒ?FKu´¤…?ïõ"Ï-›?e¡Ž
]Ù?Uºa¤ÉóŒ?e¡Ž
]Ý?ïþR¿«§—?­"±š*?*ÔE†•7?­"±šü4FGL J1451.5+1415¿ÆÄÀ†4ìÃ@M›ÑþdõMÀ:ˆÒÿì´ÊÀ<wí4Ka'@'{yž@ݖÁxô?Å{>û…i?Ò¾ä!'B@²• Ž@ë¾(DAοî‰þñã?·Ð³Œ4c¿åGªfpw¿èOø ºÎ¿àLèyÑ¿ïÿçvœ>AGNbcuNVSS J145126+141626?ï¹Xÿ´?…㣉?®?©Ü ?…㣉?®?ïøí"oÉg?`¦±Á‰'þ?LIî@Úc?`¦±Á‰"?ìü‰\L9
?¦O;ûjÑj?¸µž7¬?¦O;ûjÑe?ïX Œ\?'÷Pb}íM?"ëî~4û?'÷Pb}íL4FGL J1451.8-3851?ì;—±›Bû@2FìÔªÀ;qߐô¯jÀ<‡ªhô¶ @ þGG<Tš@gã'ñ·?Ì+ýß¿BÌ?{E"ï¥1?³\&á/?@Ùt·b}¿¦<!•.®?ï[›fù3]¿éÌewS¿Êz:ßO¿ïÿüÚ±'Þ?ïÿíÁ9ÔAGNbcuPKS 1448-386?ïñºT*FI?\YV1l'x?\‹W«so­?\YV1l'ˆ?ïÅ\
œZ?¡%\d­?}rÑú±ÓI?¡%\d­?hE–?‡pÓ¨ðöD?ŽY%þîš~?‡pÓ¨ðöD?ï¸&fƒq¦?z£[àµ?öf_#–B?z£[àµ
4FGL J1453.0-1318¿ì¨¾ôs"	@CøŽ£œQÛÀ:Ó Z8[À<Zê'-@Ô®¯Um›@^pc?jy?Ä:šE;¿ŠðÉZ7À?ÅçúîHH@ñp;Ò>&¿îPáϓPª?ڂRÀ—4e¿ìJ[¾l·¹¿Î0CÐí¿å/5B,P¿ÌT—œiW²AGNbcuTXS 1450-131?ïÝGÑ'Þ©?r€zLò-S?q\l«d?r€zLò-V?ïý²ÀÄü?Vš§z«¶?2iùØUW?Vš§z«¶?ï˜Ð–°5?‡‡ifHa9?‰ËÚ|Sòé?‡‡ifHa8?ïònEU7/?N'†Š"•?[#uU' Û?N'†Š"4FGL J1453.5+3505?âÓ'j@Oeì,äd™À:¸ŽS™ÛÀ<µ™ÙZyÉ@#>Wÿpc@X*™0¾?ÄeqH턨?²´rˆ2¿?꿹SsD›@Z(*¨3?ã¥L?ə'¿æ]4Ä,ë¿ä½Ø"kdÓ¿á»2Ál"¿ïæõ½†Þ¬?ëñø¶Ô"AGNfsrqMG2 J145315+3506?ïüË5ùuµ?5ù^d@ý?9¦P4RZ?5ù^d@!?ïý*×\¨?LRð‡y-#?6¯IEÃU?LRð‡y-D?ïه"Ì&?{\«ÀF?s<7µ™í?{\«ÀF	?ïý£3x!ã?%w•–9¡R?2æd>ðãò?%w•–9¡4FGL J1454.0+4927¿ïãݘŒ4@LÉÛ"Ðå`À;Lë8ȞjÀ<ª"Y–tK@"…|V'@¶LãÞa?Ó­Cðo¿?Ñ#l`üD4?ùìúÕÔ&@GÍ`Æi?ïõðaýK¿æÒ¬X4õ¿êÕï ·E&¿ÜjÃQ#¿ïñ'L ¿ãÈÏFúTAGNbcu87GB 145232.0+493854?ïúØlUL?LvCÓ•?GüžNªÑp?LvCÓ´?ïö>€û9?xnòÎæéW?Sƒöþ	:?xnòÎæéX?ï#º¬s?OƼ¹?œ;ˆª|±›?OƼ¹'?ïšz®²?y?;²âD?‰}þáTSÕ?y?;²âG4FGL J1454.1+1622?îÊb	/ Ø@MÒ*¡"9ÞÀ9ÞúŒ"¹À<Zjۖ"@OÞÉ# @T[òoÅ?»Ð 쉬?Å`€Þ·°Ü@žÒ¾~Up@©§°Å?í>aå£2¿â¶œLÒA¿ål(—9¿æ:m"gÙ-¿ëæíª'æ!¿ïýÝÑ×ÏAGNfsrq3FGL J1454.0+1622CLASS J1454+1623?ïÆ­J\SÖ?xHÉ. ~Ž?|©ZÑÖ_?xHÉ. ~'?ïîñC4Úh?s0@ç†ð¢?a¼Ë%˜Î?s0@ç†ð¡?î¬Aý/?šFÚíM€‡?¥;à.=È?šFÚíM€"?îø•£ÞÄþ?…6@îe*? v¥Â°"?…6@îe*4FGL J1454.1+2647¿¬4à³õÀ@O[2ßP]À;,7–oCÀ<°ÛE5"7@ØâÇàÔÂ@çÔÅ¿'R?ÆÛ Ña?¤Æa½y?Ù.$Àÿ?óT³.@?ïÉ,.\4¿º–ØÊü¿ãp,¸Å¯¿ãd¤úö«Ã¿ã îA灿Ö÷u'c/AGNbcuB2 1451+26?ïç»#Ù9¬?d5I¢Ð'°?hDÜ&ÆS~?d5I¢Ð'­?ïGlá)¶?ªe°-K­u?—cÚßéS?ªe°-K­u?ïµm"۝?'X;Þ™Ž?'¤žÉ=¶?'X;Þ™Š?ìf`ñ9e?¢0¤e.¦?¼Ìøv7LÛ?¢0¤e.¦4FGL J1454.4-3744?§—Ebƒî@3ÄüóÀ9µm¿öûuÀ;Üz¤áÌ8@ Ç†>@Ñ÷" ³Õ?ÀVË~C&ñ?É«ÿbKN³@ؖdZól@cô?ïê<´¼4Ï¿år†?tµ	¿æƒþý¡€ï¿çñLÝÙ¿ï÷Œ^G³ô?ïeÞ×sAGNfsrq3FGL J1454.2-3751PKS 1451-375?ïÆ<hà"\?ƒ(°'‡?|áˏîÒl?ƒ(°'‡?ïï¯æpJ?}_—¦?`ûPµ`?}_—¦?ëùˆ›‹?ªÀƒËS†‡?Àßá'ùÕ?ªÀƒËS††?ï´Ü#1?oÜìÍ$ýY?~¥'îwç'?oÜìÍ$ýN4FGL J1454.4+5124?îš1" @L9Âã>ÿÀ8«]|OÀ;pêWøš@"3¬?ÿ~"Ô]ºÆ?—Ù~¥¼+"?¬f¸#{ï@¹¢ž%•@ô½:ˆ'
¿Î4
H®D¡¿Úp.›ô½­¿áßÀà/€ ¿ÝâÉc`Íu¿â‹ÑŸÅW¸¿ãë[-M@AGNbll3FGL J1454.5+5124TXS 1452+516?ïýó"2M?*ñôã,¦?0g#^m£˜?*ñôã,q?ïóQT"çB?rÚݶ¼ØË?Y]VØ1~B?rÚݶ¼ØÍ?ïÐâÿòß,?ú¤¡Î&$?wŽ€ib?ú¤¡Î&#?ïù÷¾%àF?8) ;Ñ?H!h~è?8) ;Ðÿ4FGL J1454.7+5237?Àqڠ׏]@KÜýŸÓo~À;=*³1ñÀ<Ö»ÉoJ;@
—Éà´5?üË;¸<òÐ?Ô¤Kc֔!?ÝuX<8@•0¸/@9Æ7‡UÊ?ïÚ6ýÃÞ¿ín_E°¿ÈÒ<ã¶^¿äÍ _Š¿æó|†¿ïÿû˜'2AGNbll87GB 145311.3+524904?ïñþr¢xç?]Ï°J^%Q?\»3®?]Ï°J^%M?ï\ç¦ú?¬•îµ˜ã9?"ü ß?¬•îµ˜ã9?î
ܽv? w&uwçÁ?¯.¯Ò4(¡? w&uwçÁ?ê':Ùp?«-šÆ½?Çc›â?ª?«-šÆ½4FGL J1455.0+0247?èÊôŠHÉó@IÜ¡ô±îÀ;¢oþDÀ<ϓ¤£@ ïþ¾âSr?óDƒ½B(?äF
<ã?ïýfÞ"N@dä]ã
&?ô†²+‹Éø¿ïÿ¾ýq??ïÿò~#¿?9Ár%·I®?ÖúÿšÕXâ¿á*Ä>³Äé¿ïþÔãÄAGNbll87GB 145233.9+030210?ïÆw1u"µ?_֞¨k?|ÄgE=¦q?_֞¨m?ë%µÕט?Їl(…JU?Ãi(¨¡Ÿž?Їl(…JU?î–&ÐÉ\u?™=;]뿵?¦'ój8¾?™=;]뿵?àmï¬&ò?Á†‰ÿ?ß$ §³æ?Á†‰ÿ4FGL J1455.4-3654¿àúA-¡v'@3£åÙä"À:K°¡šÀ<Ž`€s@±®MÛ«@ç]<9A?ÁPrß­?™Ôco. ?ÙG…5@èe{.õa¿ê6Ù{0øÆ¿ã'^aŠ3 ¿é©?^º z¿àþ壞U¿ÝhÚÆ_ ¿ëš	`ÑÑïAGNbcuPKS 1452-367?ïÌ.2î?x9ëšX™×?yèÀfõˆß?x9ëšX™×?ïýwü
`?K[Ï(,)®?4@«…		?K[Ï(,)Œ?ïŸú*ë'?…'~îp?ˆzµEÙ?…'~îj?ïçÅ°ŒØÛ?W¬»›I*?h:Os'$þ?W¬»›I(4FGL J1455.8-7601¿é5îñ?epÀ-ñk¹Œ~(À:ÞUNæíàÀ<ß®PàÃ@ ¤£e BÖ?ýóžÈ­ƒ[?ÆÛC]!ï?¿–ºÂM¬?óËg†ø­?ýÞU·¿ãLÀmBùz¿èYõ_45¿ÍáS¨c¿á¤Ó‰p#¿Óz­%²Z¿ê>¨çë6DAGNbcuSUMSS J145543-760054?ïúàê'Lõ?=Çs-ö??D|WbÌ*?=Çs-ö_?ïú;›Lý?`OÝ°[þÖ?GŒÌ?`OÝ°[þÖ?ïçïå"i?pìŽ3Â?hrݗ8?pìŽ3Â?ï­ȍur?rŒBî°²?"ºÍÜ¢£3?rŒBî°²4FGL J1456.0+5051?ÇnPy¡Ï@LG¾ýqÀ;n=þhPÀ<œVœÄÇE@ ÿ‰ þ@Â%ĵ§?Ç;«&ß½À¿§°ÉáàÛ"?ä¾4^'J@JT·è9¿ïý»íx;?ïþ
A¢a¿¿ãARz÷#¿ä81¿ë'á¿ã¦">eìC¿¸,+×õAGNbllRGB J1456+508?ïöPÐjC¶?MTNÍ>ÒØ?S^_+x'ž?MTNÍ>ÒÑ?ïê:ö7?‹ï¢¾~?eä€Å	ȼ?‹ï¢¾|?ïØدÈö?s뛹ôq7?sö"¨…b?s뛹ôq8?ïc'cÍ?ƒkyìÁ/?"¿³Ÿfi?ƒkyìÁ/4FGL J1457.3-4246?ìGًZ@,¦‹¤ôÀ9'Pi¤ßHÀ;ú²÷8±!@4&Œ[Ãu@A¸œ"Ý?³ïîÿ–gz?¤®
aOG³?ì½7Σf¢@N%zãËí?é-¹a5$$¿ã]Ûèɂ•¿è¡ð€0<¿ä±¾>¶ì¿êhhŸ%Ë?Ëgbû!ôÇAGNbcuPKS J1453-426?ï÷{G?HŽOž «†?QË	ÅqÃÕ?HŽOž «u?ïýPý‡H3?Rq'û-ñ?5xžh×?Rq'û-?ï¯nRÊ£?ƒÎ
Ý*e?"$kMW:¦?ƒÎ
Ý*b?ïÿÁ+òr>ôUpCa27>ÿ|jÇKÒ>ôUpCa-"4FGL J1457.4-3539¿ïüEŠ•üÁ@4‰"àÀ8(¨(÷À;œÏ¥©r@f'ÿ"Û@fö^–ŽL? )¢].ü?ÅË3²Ù‡@$·ëО¥@ÓH{ÄÇp?Õ/F߸aÜ¿Ýå"ä±oú¿ä•ï ·E&¿åȖÝ&·¿ëwöaÍ¿êO'‰²›ÉAGNFSRQ3FGL J1457.4-3539PKS 1454-354?ìͼ¬€\?¸"%BÝ«
?¹'›ÿÝ?¸"%BÝ«
?ïiú_Ì¥û?«À¢: 3C?'À´k@Ø?«À¢: 3C?ë"æé¡\Ç?®ýõô‡†?ÃtdYzŒã?®ýõô‡ˆ?ïçˆßßUo?d|¸]ÛC3?hw  ª'Y?d|¸]ÛC24FGL J1457.8-4642¿åé*ó8ð@%©fàé´À:ôé¦ÙÀ<\E–F_@!¡Í­?ÿ_¥'(^?ÃÄÿa©¿¡I÷šÖ°{?ÛÌsvaÑ@ž™ÔÒÖ?ëUë#Ïèá¿àtÜ?,f?I\ÈWó¿Ú×7‰Úõ¿ç@Z˜ÒÊ=?Ðßn"¤AGNbcuPMN J1457-4642?ïù'˜_°_?Bþ5lɤ¸?I¹ž>€¢?Bþ5lɤ¿?ïù$á8‡?lÒ{Õˆ?Kãl{ç?lÒ{Ձ?ïßwƒÐÓ?xÏêE}#í?pD>–wJ?xÏêE}#í?ïÉfÍÛ?k£Uæ¿ ?{L¹@®?k£Uæ¿ 4FGL J1458.6+3722?ä:…ZN@N°hÂa9À:@±gìxdÀ<'¤@¼ˆ²@šD7guZ@§À£Éž?¸¦8ŽfàŠ?«ÎoU®2?ñÀgc¼h@
TœåT¿ê7ž&ò¿Ñ¼J^H¿á‡ÿ¨Â+‰¿ä'Ôôó¿Þ@°ÿç¬L¿ë4o©GhAGNbll3FGL J1458.7+3719B3 1456+375?ïýr×Éáð?0PÔ?4iA°ðw?0P²?ïýֈ8Ã?NÒQ"í¼A?7)K¾9èL?NÒQ"í¼F?ïÞ6^÷8?t1/ê£î?päôP"d[?t1/ê£ô?ïú­h¬S"?4Æ
1QŠÚ?EJ]N±ë	?4Æ
1QŠä4FGL J1459.0+6129?ì=É9'¯@HÊnÁ~ºñÀ;NéH-–;À<ïóŒT6¹@£À"'Œ@þú¤vln?Ã¥tU·B¿š³ ,Áæ?ÔçñìA[@$»]Ž¦?áú¹¿©Î›¿ã1bV}¿å/áoA¿Ü˜/w便êŸWH¼1t¿ïêøÒU-AGNbcuSDSS J145852.69+612813.8?ï²–.{r?{œãƒ.'?ƒxšta#¾?{œãƒ.?ïí'gP0?~øOzl^Ê?bؘ¯~Ï?~øOzl^Î?ïœ^üû?…#g'^Y?ˆèX˜€ÁP?…#g'^Y?™uU?tHüˆ 'ô?ˆ›¿¢ª§?tHüˆ 'ô4FGL J1459.0-5353?è‰ù"§£@Ú\ØH+À9½òJ·À;Y^Sô@§ÔNKg‡@Ն¯²
?ºÒ]Ÿ1Lî?Á$xFÜ?ò͗b‡´•@<Yÿ$㺿ïøe˜º?ïû
H5#¿ãší!*È¿êµg £#0¿å$WÞ8Z¿ä"%B{¦AGNbcuAT20G J145935-535047?ï\ÄE£7?™€nԙ Î?"gwK™?™€nԙ Î?ïQÀß"yÆ?²dùxØ1Û?•Çä°ÇG?²dùxØ1Û?ì
¥!e$H?²{ëöMÀ?¿'ÖôÖÝÀ?²{ëöMÀ?îˆR´}?"6ܐí?£Þ7zÔ¸$?"6ܐì4FGL J1459.5+1527?痚¼ÑÀ@M
AÝ!êÀ:ÿ@Iœ+DÀ<œÑ*)Ÿ6@*èãXÕ@Â|ò—?É2.3o?¹y}†8ê?ñ%õ'^éš@p½Úìu4¿ê¼$ô?ï‰ñ Á¬¿ÐÏ(œ¬Hž¿Ü^IA<‹L¿êÙ8¶)ó¿ÔvOýï.¡AGNfsrqMG1 J145921+1526?ïü¥ì#¡¦?9!_Š²SM?:ОâòÜÇ?9!_Š²SU?ïüdþ?S&S1žö?<ß Ð<?S&S1žý?ïö®—È?>ñw:?'\Z?>ñw:"?ïâãûI*}?^,Ð¥æO?m¶Õ'?^,Ð¥æNü4FGL J1500.7+4752?ëÆG4Lj@L¶°hÀ:VL¼q4÷À<Q¶3-Sö@)´½atå@‰‡á
qs?Ä<37
à?ÁƒxǼî?ûúí!*È@|è7"î?áV.	þ‡¿äåܝû(¿âØr‡ÜØ´¿æ- í¶Q¿êÌ_iœý¿ïþ·`Sý®AGNbll3FGL J1500.6+4750TXS 1459+480?ìùæń{?±|W;‰ˆ?¸3ðÉÓÜ(?±|W;‰ˆ?ïkŠ™û?Ÿî¡!V«?'Ž¿^ŒÀ©?Ÿî¡!V¬?î‹:$},?›TVB?§OŒ]¸-1?›TVD?믎ýlÞ?£åÅ3¤e?ÁC©Ä
L?£åÅ3¤f4FGL J1500.9+5528¿Ð+"÷@J¥éᰉ À:ä¸qËõ6À<¹ªYÛ=©@oœÅóë@qޟ]'ù?Å06(°ù?ÂA!"µ?üê®ñð@#zÉIàt¿ïôL7å?ï¥~ª*
–¿ß—ºò.Ü¿ÜÕR'XàA¿ëó×"f1b¿Ó$e$œíaAGNbllFIRST J150106.2+552750?ï¬.×Ú­?…ŨF14a?"ôJ<ITä?…ŨF14_?ïóæÔ3?pˆléòß?YÞ2W՗-?pˆléòß?ï$ØôI³Ö?"¢FõŠ?›dávɅ'?"¢FõŽ?îéTH¯P?Ûáu8?¡j»uªý?Ûáu74FGL J1501.0+2238?ïûÚ^p@N,ý\·ûÀ9Å㤀À;ýåﳁ¢@úÌx"n?ÿÆ·	)?¨Ì7Tüº?­@
ÿYß<@3Xz™@ÄÓÏöLù?Õcä`è"¿Ûžœ7ً¿Ý©aùDO¿ß¨"í8¿ã
O¿…ç`¿á€`•AGNbll3FGL J1500.9+2238MS 1458.8+2249?ïþÝ!dx?$/â£ù"­?"-é¸5?$/â£ù"ö?ïùtÌÀœ?^‰\$
²;?J,ÏÄý‡?^‰\$
²6?ïæƒAQwv?rp7²*s?i|¾®ˆ‰U?rp7²*s?ïñ"%öR?I+ô½'ý?\×µî\,?I+ô½'ê4FGL J1502.5+5552?®‹ëú¯²ÿ@Jo…¸QìÀ:_sN¬5~À<}}Ž¡@…×x¢S'@ú <¶i´?¿0'ùD?Ã=ñÓ'é@ 6^`Þg@P±šÂ?ÏݪÀˆpÒ¿Ýz\9â$¿çEb¹2¼¿ãecœ‡Š£¿çªs;`ÿ¿ïüç|{{¡AGNbcu3FGL J1502.2+5553FIRST J150229.0+555204?ïé.È[{‰?zDCñùq?fÑ7¤"w4?zDCñùu?ïü'%Ca?SŠÓXYÀ?>ÆÕä÷Áf?SŠÓXYº?ï"@-»"'?†)¦O+î
?‹/ô'6?†)¦O+î
?ïê¶w,v*?P¸µ½Ê?eIˆÓ‰Ö¾?P¸µ½Ã4FGL J1503.3+1651¿æòƝxö@Lï9C¬ÅÀ;4<ËbÀ<šáìÂo@ îÐ,Ӟ@Ü¢Ûa»?œ{á¢ÇÁ¿¢Ø€'y©?âU/<-­¸@³ch…$˜?ïÜe@Ìxê¿éÈLŸëÃ2¿æõ=Ïng½¿æ±Ï»"–%?ÁuîÚÛz¿âp· gAGNbllNVSS J150316+165116?ïø]UXŒ?Gö:n¥¬‡?NŠ«úÑ³?Gö:n¥¬"?ïû暝?b— ~2p?Be–‹õ?b— ~2n?ïÛÇ1aÛ?ve}*›?rwœgOy?ve}*›?ïæmÀ\kª?`:¼"?i'?£"W?`:¼"4FGL J1503.5+4759?çý!w;@Lx•¿ðExÀ9²amaÚÀ<I핚0˜@ÜB4-@"j㣨ç?²âÚÖ$å=? Èé_Ìæš?ï
	žs`@	4\Ç×­¿áÛÆ«±Ê¿ßێ0¯Ë4¿ä?KâCW¿âyÃ:|Ô¿çhƒweR¿à"¯\y}šAGNbll3FGL J1503.7+4759TXS 1501+481?ïøë@؏?Bº'â?"?LRüŸ¡Ê?Bº'â?"?ïúÖª°ï?YˆÇ‹ˆÝ\?D¥U<CŸ?YˆÇ‹ˆÝ]?ïî­»!Xþ?j@KB5?aRDÞ§¶?j@KB8?ïÒF{'
G?fdÃËÊcô?vÜÂ>úÜ+?fdÃËÊcï4FGL J1503.6-6427¿èI‡\"'À"{¦iŒÀ9‡B,Ë:&À;w›9¬Éø@äuÚ͖v@¹NþjԊ?ÀÓbDé?ÁŽe³ãó@
žá×öÌ@
¢¸ý0?ïêž‹¥»?ĶúÓpTý¿é°Oô4ã¿â1i.—ÿïøÛH"?ÛmNâçxAGNbcu3FGL J1503.7-6426AT20G J150350-642539?ïl'»Þ[?•pùÖ|+?'o¨4º?•pùÖ|-?ïùÜ*üۉ?fÎyd
ô?HT'Ú?fÎyd
ó?ìü•}¼;?§˜uò")X?¸S|/?§˜uò")X?ïÓCv˜Ë0?gŒ<õw½Ï?v^D³šg ?gŒ<õw½Í4FGL J1503.7-1540¿Ñ
)€
Ôt@B?ÿñÀ9GúËã˜ÁÀ;Þª; g@ ~fpâ–?üLû[V?°ˆà <ó?«ƒÛÂ3?þÓðÈT˜@P†èçày?ïáŸØwü¿¼†ˆb¾¿àÐ^¼>¿ÓÙÔ½\¿Ýt§¼òå¿Öyɺɕ
AGNbll3FGL J1503.7-1540RBS 1457?ïòÄ'Ì9?Y‰/'QŸ?ZwÂúg‰½?Y‰/'Q¦?ïñ"i™K?sZ¼Pa¹?\÷Å,Ím?sZ¼Pa·?ïÕµ'Š?wuQ³l?u@%lu»x?wuQ³w?îÛžWÐa?†ÖOÃø?¢OÖ'ùô?†ÖOÃø4FGL J1503.7-5801?èZ
X?ݦ‹D—3¹À8%ª]6;üÀ:Dã¼ÓZ†@BÞS\ôM@ÔxþŸ3?³ ~Ôá?ÒL''ØÛ@!€¿®Y?ïî‰ÿó–?íœtà|¬ú¿š¿?#49¿ã§ÿT0¿è%d=—:D¿ëê¹FÞ
ã¿éý¿è,AGNbcu3FGL J1503.5-5801WISE J150334.23-580119.2?K'º2)¸é?J¬'¹¦?ïù6su'?J¬'¹¦?~æ-ä¸?'÷92u:?ïÂ3¤6ç?'÷92u9?ƒç² Í?rà⚛"?ï°c'7|Ë?rà⚛8?)st¯hàU?EóB}Å?ïþhȵ	s?EóB}Å4FGL J1503.9-4247?ê"!،@+k{[À:5âÏòÀ;ý+ÐhbÀ@‡[ÿZ>@O¡—Zû?ȅ#ÖH÷k?Ô©Äõgö‰@^n<ô}@ITݧæ¿ïÿýFKê?ïÿÞý¦ßR¿å€èÈ«ÕÜ¿è>¸c­O¿ïþ³íQ¿îv¹?|AÅAGNbcuPMN J1504-4248?æ°;"~­?Êì¾å"LŒ?ҟˆ×Þ¦?Êì¾å"LŒ?à¾ãztØ?Ó6/Ö~V?ނ8ßO?Ó6/Ö~V?ܵpÜâ ?¹°¹)ö?á¥G'Ž°?¹°¹)õ?àƒS%-Ê?¼§5K`&°?ÞùY´ß¤k?¼§5K`&°4FGL J1504.4+1029?Øb—úÌ>@KJ¥ß"9çÀ6Uü6GÀ:ð·E|@á9Q/r‰@þÆDƒ?€OH¬[?¹>àæ_E
@1`m?ž{@#MG0– ¿ÅiÌLtM¿ßzûÿjXä¿ämÂæ™ým¿ägHÐöR¿é:®ƒ¿ëŠ7KšAGNFSRQ3FGL J1504.4+1029PKS 1502+106?ïØ3(¹Úû?l¥J'±}é?sæk£'?l¥J'±}é?î"ê$ÿ/Ÿ?¿8«)·?¦Á]°
õ?¿8«)·?ï –"zÝ?–õA–Qš"?›í-p¤\´?–õA–Qš•?éc™Ûº?ƹ*¾}Á?Êq˜"¹ð?ƹ*¾}Á4FGL J1504.9+2027¿íEehnì@Miáâއ	À:'èYñ
À<q¾7Ô
@•)h¯@¼l}ܟ?º8yÄ<¿£Š~•?åtU!š"{@ñm@U¿æ°,X¿ã8Zðž´¿çu\}ÚKf¿áÕë#Ïèá¿ãކžR¿ïÝ€ÙYAGNbcuNVSS J150503+202811?ïÞ_`)Q?fS)½ªÑ?pÐOë|×1?fS)½ªÕ?ïûA=ŠÒ?VEAèþM?Bû	ÉÔ¸+?VEAèþX?ï¾üs—ê?|×ýɑ§?€@ã\Ö?|×ýɑ¡?ï¾ÜÀE³±?nqó¿ØÓ?€HÏî"Î?nqó¿ØÔ4FGL J1505.0-3433?ݕkQÌ߂@4°•9¸ˆrÀ: ¤¸±À<;2U½¡·@"¨¢J˜@…êZ|MX?À3ˆX(¶?À êæ`G@<9ҍ×@
†AÏß?Þé;'¦†?ïâӟNå@¿ä~IÏÞ¥¿âX»¸¨Rš¿ç
z!¯'J¿ïÿœb¡µÈAGNbll3FGL J1505.0-3432PMN J1505-3432?ïã֑É#Å?kFKÜäö4?l)n6Ü:¸?kFKÜäö3?ïõTEuvÍ?na=dÔË?UWuf½?na=dÔÏ?ïV>L»"?ˆyØýg?‹êplÑF?ˆyØýe?ï¸Ôo
MF?pßrÆ?Êä<¬®n?pßrÄ4FGL J1505.0+0326¿ã¥í@@I!lœ
"À8Ó§óÏpÀ;ìнU¡@;Ò2¸@ê¬azŠ?©ˆa97??¹^èî–v$@`dÄ¥¶Þ@/½É¤¤:¿Ð"h<ªUT¿ãµ´ÂêÌ¿è1¤½º
R¿èšc"åV¿éœ¦š3¿ïÿrܖnlAGNNLSY13FGL J1505.1+0326PKS 1502+036?ïúÕãHc?@""Í_|f?D«ÜrÞw5?@""Í_|x?ïôŽ—à=‡?s÷ŠúÁD?VâÐ?"òï?s÷ŠúÁB?ïšH)	{r?†Mm'Ž¤?‰mõ½¡#V?†Mm'Ž¢?ïԉQú€7?fOUPþè‹?u»W¿äk?fOUPþè"4FGL J1505.5-8241?éÆOqœ~À4ú9櫛$À:¡Ñ'¥`wÀ<}kgW'.@ >K¶··'?ÿ¤;~[O²?Âsýiw¾?©/†DA\?é«ù®ro@ïÒÇÄ?Ä4<»Ív?Ë*ž¤›U[¿Ó=Ž >¹Ï¿äXý'«Æ¿Ó˜úìð¯¿ä*[…~AGNbcu3FGL J1504.5-8242WISEA J150525.41-824231.1?ïìÚêÂV?`
ë³õ}L?c%æ=«?`
ë³õ}K?ïý•Y߈?Ncù ¹D?3U1¿l!?Ncù ¹D?ïÊ­Þ¢»?lò·x¢?z©v®¢ï?lò·x¨?ïلÃŽI?`yV/×¢?s=±8Û¶?`yV/ת4FGL J1506.1+3731?غƒ¹Œö@Mó'=[«"À8nd"ÕÀ<3mÖQ@D`%Z@/Þ|·â?Ÿ'†yù—?ºA–{@GՁ§4@Ÿ¶'³y¿§¯Þ™AÊ¿ãÑél?Ä;¿çO'ðßь¿ç¤8#\üZ¿ë=8À:î¿ïþ½	á*RAGNfsrq3FGL J1506.1+3728B2 1504+37?ïøKÙD8s?GÒ¬ÉÔÙ?NКï5?GÒ¬ÉÔà?ïï ¨y'o?y-Ïð¡‡Æ?`ßW†mÔ?y-Ïð¡‡Æ?ï¥üŽ5wc?†Sâ¡ø3?†€Ür¢&ë?†Sâ¡ø2?ïþúÙøK?´RÄý~`? Wâ`{Y'?´RÄý}æ4FGL J1506.4-0540?á\˜nÿÌ@Eܺ`À;{kà"êçÀ<ž`·Ð¼@"ìr'9Õº?øYÙû‰xº?×\ýç!?Ë©=¦~¯?ñÉa=1¹¶@/ªÁŠ$¿ï')` §¿ïéMcÓ?ï÷3¨£ø˜¿×§amÙ!o¿Ç<ú\Rn¿Ó^U`Y±øAGNbllNVSS J150637-054006?ïüńý1?4ĒÔô?9ÓØw$£?4ĒÔà?ïý{d›¨;?Kó·7[Ç?4$Û"¾((?Kó·7[¼?ïÙ ì†ýÔ?sãD€:®?so‰¼à?sãD€:¼?ïògŠ?R·ÃVÏ?[0ýÙàéG?R·ÃVÒ4FGL J1506.4+4331¿éøxý¶É@M!ý`éNäÀ;CEћh§À<˜&B‰èL@xU'¾·@¶ŽYÊv±?ÃٙycCF¿§‡¾د?äöóaŒ@ö^KdØG¿Éà ¢6÷?îÁÿiW2¿âg`âC±¿å‹	H~¿â3''d3¿Ü™špY.oAGNbll3FGL J1506.3+4332NVSS J150617+433413?ïÌ#'GÑ?y‰ò¶t?yî>ü\?y‰ò¶s?ïûƒ¥…ɱ?U4ÖoMØ?AñièÙ?W?U4ÖoMÞ?ïF܌®"?"k•7#?—?Dnj/W?"k•7#?ïÇùn·?my©ÒW‡?|H¤tzF?my©ÒW‰4FGL J1506.6+0813¿èvK£¨w@Jl÷ µíÀ9_N"¢Â7À;ÍßgDX@¯T§¢ò?ùŽ%)/?³¥µ%ç?¼<©>'X	@—ƒ>äA^@Û¯fœA¿Ü]ÝÙ¥¿¿…	ꏀf¿ÓþuÜ{ ¿Ô!}Uì¿Ý²ú"¯tÍ¿ÜÞì>Ø
AGNbll3FGL J1506.6+0811PMN J1506+0814?ïüât-‰R?53=!?8ì^"µrz?53=!
?ïùYǯ¾?Z«·@›:?J›èáAS?Z«·@›5?ïÜ×Ižæ?t…
ÃTV?q"[0Œù¸?t…
ÃTV•?ïÍïtžL?b'u'8'Z?yE°ñÙï?b'u'8'Y4FGL J1507.2+1721¿æ½«OèT@L™£!h0À:‰\qÀ<Wκã–=@ em¿öûu?ø‰Þ¦$ ?Ä/g Ë}?Îæ|¡;N‹@¹A|¢@	ت•yµ¿ï~Å`?ïp?}ÄPý¿©×!~CÁ¿×ŸlAqºW¿Ò`½§?õ¿ç"T¼÷AGNbll3FGL J1507.4+1725NVSS J150716+172103?ïî•<Ä\D?_Zæ#I?ajÃ;£»?_Zæ#L?ïøӂ½?b=‹¯<.?L±÷Ñ	Œé?b=‹¯<,?îmwÍt&?ŸÎçü;¹?©.ˆƒ(½°?ŸÎçü;¼?ïÂU
-P?kM$wBÚ?~ÕzÿiWy?kM$wB×4FGL J1507.3-3710¿àçTñ;üÎ@25ƒƒ­Ÿ
À:_'j@À<L$s|Ï^@̤.Èë@wÖޞ†h?ÂXê§Ôó?ÁG֘Óv	?ýœ¹ßŠ?@W?Ñ&MÈ¿ïÉU^?±?íf.¢<Ö¿è]œ"I¿ÚébÖ#c¿ä%ßøù{'¿ïÿï¿@PAGNbcu3FGL J1507.6-3710NVSS J150720-370903?ïYN	™´í?›M˜Pë?"Ö>ÌÉb?›M˜Pë?ïs@Šg5?ªGTZöêÚ?'—îN³g?ªGTZöêÚ?ï=Ø+éž>?"µGÙ®]?˜Dú'Ì8l?"µGÙ®`?íãómЯI?CQy]?°àd'z…³?CQy]
4FGL J1507.3+3341¿êÏùÿyë@N·=CÀ;1@À<Ïâù^ü@  ¿þˆ1?ø¸¨RšÈ?Ó­Ü|m8è?Öõ·ý‡Õ¢@f݄ªõ@\[J©q¿ìiþ Õ®¿ïæ»@2u?ï›r·­¿×@>Æå,¿áp¿ïÿ⾦™\AGNbcu87GB 150531.0+334938?ïøA×Ò÷?G4Ÿ…?Nø ´''?G4Ÿ…?ïù†Tð?`¸ïq.|Ã?K™çš¬>³?`¸ïq.|Ã?ïx'~‰Ï?Šqq]ʑ?û.Æ™?Šqq]ʑ?ïróó·Çr?ƒßŠ'§?'¡‰¹?ƒßŠ'§4FGL J1508.4+7717?ätjž/_–@B¬ÜY1ÊÀ:ò¦WíýŸÀ<ã™hò1á@c`í*»@,næg¨†?·ž¹¾þ$¿µÑž~ìÖ>?úáՍe®±@‹Í(<_¿ÔǙœž±±¿èï^¶¿â—À%çñ¿áž2OÞd¥¿áüE°ä9¿Ó9ïô8AGNbcuNVSS J150811+771819?ïüŽ»žbñ?4/l¹ÈÈ?;Š#èu?4/l¹ÈÃ?ïýzíÛ©*?M¤žœOµ?4('"¶¦?M¤žœO´÷?ïç¬KEVÒ?vl‡ã»ßŸ?hS´º©.í?vl‡ã»ß˜?ïú[qG~ì?3ç¾2}3Ô?F':âS,?3ç¾2}3¬4FGL J1508.5-4951¿åã~J·Ed@Ò´|lbÀ8´"}Ðæ7À;; 'oÿl@œY®ê@žÚH¶R?²5Iè‹o?Ō¨Å["P@sœcxu@–,ÞZi?Ø¢@\;•,¿æNI¿ê5`Iô¿éF3 ÁV!¿î 2:ïÿóÖ&ãAGNbcu3FGL J1508.7-4956PMN J1508-4953?ïŸÀ@—p?"ç©çݤ?ˆïÚ#ÿ‡?"ç©çݤ?çgÛ5+{?Ó¦ýŠÙ?Ñ0I•©ý
?Ó¦ýŠÙ?ë¿ØùyV—?«û"w{Ÿ?Áœ¥¥?«û"w{Ÿ?ç….j€'?±wdZ?Ðõï£*þÝ?±wdZ4FGL J1508.8+2708¿ï´™ô"±@MÄ6~ANÀ: $-ÿîÀ<Rv‰Ê@~ÄN##œ@¦M™æÆs?ºâL¤>Ó¿¢F—'×Ïú?èŽÙ·–Ú¢@5ù¥ž?ïìh ¤Ñ¿ÙãºÚ±çÄ¿åëÍ
dl'¿àSÞ9ۿׯ͸…,¿Ôá,Ö!à%AGNbll3FGL J1508.6+2709RBS 1467?ïï~u—'ÿ?Zïíº"Ì?`Šhmå?Zïíº"Í?ïùbg??^œ¹o÷P?Iúvcç©?^œ¹o÷V?ïã·`0å?q0ތR‡r?lHŸæÏZ?q0ތR‡n?ïA>¦ˆÜ?zÐ^Ù£-?¯°V]ȵ?zÐ^Ù£.4FGL J1509.6-4334?Ý'åš–@)Íl.ýDÀ:êHޖ#À;á•ÊØ@Èý4s¥@¡íý¬i?Ë|,Ñð"?à.Ò`Š"S@})Àµ@n埬ƒ?ï¥(xÅ
¼¿â¤9/Ìvf¿é½¿ÚËé¿é×ñ=Å]m¿ïÿù_|è3?ïg4ø/Q&AGNfsrq2FGL J1508.9-4342PMN J1509-4340?ШYY,š?ɱŒ°:u?ç«ÓSi²¾?ɱŒ°:u?ÅЗªL®U?Ì{}…ÿäz?ê‹ÚlÔk?Ì{}…ÿäz?ÖFÖžÌË?·õb;Az?äܹ°™›?·õb;Ay?ÆwÙIê®?´Ÿ#RƒS?êb	­…x•?´Ÿ#RƒS4FGL J1509.7+5556¿çÆÔ\ÉÊ@Jo~=ÁÀ:@K!JÓÀ<ŽævÁþ=@ 0@	‹€?û÷.?½iSWjö?ÀD,?Nœ@Z'£S&?üöèˆ?)?î0Sà&ñ±¿æ·'I%E¿Ý2;;•Wk¿Ñ¸䓒ï¿àñ¥"yŸ(¿ë'ž^ÿëAGNbll3FGL J1509.7+5556SBS 1508+561?ïá:žN>ç?fø+´©÷?nÅa±ÁÇ?fø+´©õ?ïmìwyšÄ?¯UÈNä·
?'Bq̧r?¯UÈNä·
?ïŠi²OP}?Š0uGyG??e"l+á$?Š0uGyG@?ê¶!"õ£?¥;÷Պ?Å'y°+ás?¥;÷Ջ4FGL J1509.8-2906¿ïÏ_ç‡@8¹yŠ˜À9'[4<ËÀ;ùÙLJ®@Rü'G—@3n<½€?¸'Þ½?ÁÇp×ÙpI@Š.oKè@®w!I§¿¨ëÂlÕ¿çòÖKÒ¿é0]€c½•¿èœPbîâ¡¿ía¬ÃB
¿ïö¾7ޓŸAGNbcuAT20G J150945-290502?ïñ²0*x?Zâ¤oPŠP?\šáŸ«?Zâ¤oPŠP?ïûFņ'?V¤½IÉ?Bäéçc"Â?V¤½I¿?ï'R?ÉÝ{?ƒû¿ô±û?‹kp
ˆ¡G?ƒû¿ô±ú?ïÒoKߖ0?dX¬ÕéG?vÈZ4è?dX¬ÕéF4FGL J1510.1+5702?àÕtósÞ@IªB¿˜0äÀ:¢<g[RÀ<ª4òP@¸ˆå—I@
4˜?½€žöЬU?fmȁúƤ?¨á߯\Ï@ú8õêÓ?å4ªÌÇÄO¿çvÇý°Ž¿ìܽ¹‰y¿å/hۋ¬¿än,Rn¿ïúÎg×®AGNfsrqGB 1508+5714?ïúÜÎþ#?_ °½"?DŒÇ´v?_ °½"?ïü熁+?]Z''ãË?<ÃËöšZ?]Z''ãÊ?ïÓ±ôîú¶?{bWØÚ?v'ˆ'¤œ?{bWØÚ?ïõNÎ#œ?FÐ|…&#?Ubc¹ÒÊ*?FÐ|…&4FGL J1510.8+7959¿î¶ª'«iT@A•¥CñÇXÀ:ßB¶]õÀ<êž…@¿kÅöÅ@Eʯ¼Î?Â(Cg2ê?«
jØf?çù4j¤9@êÓ_Ž¿ç4yð'Î?ïî6¿Yǝ¿çD{û#!m¿Û§˜€|¿â«5£OûÁ¿ìïÐ!ëãAGNbcu3FGL J1512.3+80051RXS J151026.3+795946?ïþ®£È·u?$ˆé•ì?%ÃtˆÁ°?$ˆé•'?ïý bcQÕ?H½\7ðê™?2üìåqV?H½\7ðê˜?ïäq[&
?rd‡"?kŽ¤Ùñö.?rd‡?ïÿï}&@?iü?ˆE?'[8'?iü?‡4FGL J1510.8-0542¿ÝLÙè@Eyùa€M˜À8ؔqÌÀ;"
ɇï@["Ì´@71½è?©°åæyF=?¼¼"Ûw4•@YyámmÂ@P¡ú'+6?–ž=¿Ò¨˜Â¿åÇ#ªÿók¿ç;,%ø¸
¿ê¨¿;ê'Ú¿ãkÀx*´	AGNfsrq3FGL J1510.9-0542PKS 1508-05?ïâÃðÍ?i -Û7¿?mþô<4[?i -Û7¿?ïëëjqr?u²Æ':Û?d•ÿŽŽÕ?u²Æ':Û?í­ˆð¨¾ä?¢}Éí‹êË?²"¸zºß?¢}Éí‹êÍ?îõzªdÎ`?…M^ÔS? ¨UY³?…M^ÔS4FGL J1511.8-0513¿í¤us`´@E[|þX`À9‡ž ç×À;ò鳍a@ ‡øø#è'?þR@ßÄ V?¼FHcÆùÏ?¨ã^^°¦?íé"89,q@ŸâÈÇ߿Մ'!W¶¿è¥žTê= ¿æ\º:¿Ç᝿C!h¿áà¥â}8:¿Ú}çAB?–AGNbll3FGL J1511.8-0513NVSS J151148-051345?ïø"g™k•?Gâê$¿­ð?OvašQ­ë?Gâê$¿®?ï÷ÃʘdF?h¼¾7W'ô?PxjÏ7qù?h¼¾7W'ô?ïÎ
Cè?}rŠh{]?xózÞ¸µ?}rŠh{^?ï™Ciõ?wI£oF€?‰¸ï%˜'<?wI£oF~4FGL J1512.1-2255?ÖWÅhø'@=~"î9.À9ÎޑoÀ<!שŸ¡@ 	øF£'?ýü}ÿà?¹‡5híJ?³ŠJq=Yþ?ûmAfҜð?ü=aèRdQ¿ÜŸ9`ô·w¿Ô¿eÛüëy¿åtïËÕV¿Ó'vû	 :¿Ûî›ÿzt¿çǸƅŠïAGNbll3FGL J1512.2-22551RXS J151213.1-225515?ïãùBïBÚ?dæécŠ°?l½½%U?dæécŠ°?ïµ$‰Ž ?An?'¶ÝœWÛø?An?ïŸ%/.£X?…%ÏHZ3?ˆ6´4W*C?…%ÏHZ/?풁·¾?—®S%ò>¹?³kózB?—®S%ò>¹4FGL J1512.2+4704¿ï6×<'ó|@L>}QÀ;6©ðÿ±üÀ<äæíàBË@.KAò¿@\Ôí,¿?ÑqD:íg?³#uÐ玚?ãŒf«/Ä@E<O'²¿àdy¡*]¿æˌ%<Ðk¿æ¦j±N¿ÔyK%BY¿àÐI ]¿ïÿç@ìYZAGNbcuB3 1510+472?ïÿhUqQÝ?ց†‰Ôí?õQÕÄgç?ց†‰Õh?ïýØå?RÔrê?7)?wøéŸ?RÔrê?ïóºÕP%?fcg°'ä+?X‹òU_¶?fcg°'ä3?ï÷¶À?@üEÅ??QÇÎz'~F?@üEÅ?/4FGL J1512.2+0202¿æOâiÊO"@Gý›#ÝTÚÀ8Öu£KÜÀ;ɑÆf>@ÁX';§ ?ÿ~Ö|¨È?ªˆSöø'?Ä'q¤€¨@#'\´5ý@SOÄ +¿Ùw<!™X¿×Du»Cš¿àþ‹ Z›¿â¬×cÿƒÙ¿é']ýa?5¿év%@OvAGNfsrq3FGL J1512.2+0202PKS 1509+022?å¼øà"sk?ÈÑéêºÒ?Ԇ>Ù)?ÈÑéêºÒ?éîSá˜Õ?Ñ\úÉq?ÈG¾°yœ°?Ñ\úÉq?ê
GO?²>žˆÄ?ÇûÖâ÷«?²>žˆÄ?Þ}6¯Ã–?µ\O]S4?àÁd¨4ö?µ\O]S44FGL J1512.8-0906?êí&=Ýbg@DËÑ$JbÀ5˜A‰7KÇÀ:k' ÿT	@VP"&ë§@òa|ÚQ?ƒÍ#Ç?¬ƒÖAsE{@'ö«ÿÍ«@!`&	ÿËÄØâ"Äö¿â'\f2d¿æÉÁ/á¿åŲÍÈ¿è2­œ…Ý$¿æð _ñØAGNFSRQ3FGL J1512.8-0906PKS 1510-089?íu5Ug~Î?¸(µ/fÕz?´VUTÄ	ƒ?¸(µ/fÕz?ï°ÞcbPv?¡ŸÊ–_n?ƒÈg'kâ€?¡ŸÊ–_n?îp0:v²¦? ü+ñ(C?¨üüX"Õ'? ü+ñ(C?îêfø!2?™_Æ«ÂJ?¡^i}ìç?™_Æ«ÂI4FGL J1512.9-5639?ߐÄ×è´?ðg¡á^TÀ8Ç£è_ÐÀ:ùҍ.#@T͆=,@dÆS6?´Œ4қ?ÇSy9QÛ?@àþ}=C@ÂÌ«êª?ïÿp\‰n¿Ð
,"óŸõ¿ã¤"CÆÿ-¿ß.ß[Å£Ž¿çIú?KÅP¿é·}z"AGNbcu3FGL J1512.8-5639PMN J1512-5640?ïےÁ?wà…Ž‡(7?r6Ÿ1¨¯?wà…Ž‡(7?ï»Ó=2ç‰?¤Åä¯êü?0³F€?¤Åä¯êü?ë¾ÉœœyÄ?©'9£ÈL·?ÁٍŽò?©'9£ÈL·?ïÈ:~LŒ_?j•âõõ&j?{âÀٹД?j•âõõ&o4FGL J1513.2-7131?íg¸$–øÀ'c"ÀÀ:´Ôˆ'ñÀ<Wi¯Çˆ@"y¦	>˜@š"ÛÍÐ?Ä<yX¦?ÎcÜwµ@	£1…´	‡@«	¼Ad¿Ð(³"í?ïþ'ö ¿ãotâ«}¿àhþ&,"¿éU¯"­¡Ž¿ïÿÊñ*z'AGNbcuPMN J1512-7131?ïÝ0ôK&?uöˆZ»¢?qg…Ú9lö?uöˆZ»£?ïøÞIk~?jÒ-»Ö|?L†ÛšR'?jÒ-»Ö|?ì¢Py•Ö?¦žiEf?ºí|3QO…?¦žiEf?ïøeâÅøè?AX¨ÁÚÈ?Nhtècg?AX¨ÁÚÂ4FGL J1513.4-3721?Ú '™…@1h²ú"¯uÀ:b寺À<O)1Q±£@"®ˆ"
¿@˜säÔ*?¿ÊgþÓw?­¼³Ïû«?ñÞ¦éä5?ûŸ5åÀ¿ïo.áêÁ*?ïì¢À‰Èk¿å»àì>'¿àð™Ã¿ÞËrÅz%¿àpÊ"M‡ÈAGNbcu3FGL J1513.3-37192MASS J15131867-3720114?ïâl³Mt@?h"X¸'âL?m"L²‹¿¸?h"X¸'âJ?ï`4©Åb?¨áðÖm{­?"ùjÇS½É?¨áðÖm{­?ïÕ¿.A?vŒÉ@د?u hýyÞØ?vŒÉ@ب?íè=·Àø?œrjI•¯3?°¾Aÿx;?œrjI•¯34FGL J1513.4-0753?é<–O=V6@DuáC|V"À;bˆRIxðÀ<‡çQ³Pû@"/c¤• 8?û§+y*Ž?Ò=ðüVþ?±b;^zߚ?ßÈ*[sCD?ö-.vàÜú¿ëBĀx
~?ߧnƒì3D¿ç+m´Z濾9HËö¹¿ïê[ãU¥?ï²Ã×ZÅHAGNbllNVSS J151324-075450?ïý*1R|N?8>Oq‡?6®ul~?8>Oq‡\?!MB?·IâÄÙÏ#?È~ÖWÖ?·IâÄÙÏ#?ƒAyÕ?…0¤Cú?¶?‰[/¡Šx?…0¤Cú?³?î`5š öÕ?¢ù XÈÞ?©ü¦Uð'°?¢ù XÈÞ4FGL J1513.4-3231¿¹O•[™_´@5r›ÏÔ¿
À9v)a"YÇÀ;¼GÜ7£Û@ÛQv?Lq@á#ôÑÏ?µÀÈ\¥?Á•T{ç@ Öoþ@û0$
 j¿×9Fr«G¿åSFÎñj;¿ä›Âhż7¿çè0Àè#¿é{'{;
¿ïÿû˜'2AGNfsrq3FGL J1513.5-3233PKS 1510-324?ïô¸ˆCÿ¹?S\ûÆêCx?VŽïxŒÝ?S\ûÆêC‡?ï÷–õa»?n¸<Þ¨®?PÒ<‰Ë€?n¸<Þ¨®?ï]vÏBdï?Š›¨YÑ¿Š?"Q&³b ?Š›¨YÑ¿‰?ïûˆS(Û?1¤°zƒ6ž?AßÒ³\""?1¤°zƒ6¡4FGL J1514.4-7719¿íu#2ãÀ0¥Ì·ÔDÀ;ǀ¾/À<àÔfõŸ@"á%T"l?ú)'jÑ/2?Ñ°Ëdlç	?Ħ–—±?ó¥@Ìxé÷@åÕÑ-Yª?ÉðXC=—¿ïÃh4œ¿¿?ïëÇkcü?ÛCå½´€ü¿îHFøã?獨eÓAGNbcu1RXS J151448.8-772249?ïø^"fÜï?L‡OCB(þ?N…²dŒC:?L‡OCB)?ïü‡Dø5,?^'BUpW?;ÅØ>Vž"?^'BUpW?ïrŽCµ×?Š{ˆ‹?'®7‰_åS?Š{ˆŒ?ïéÀb6ùá?gsµ×z_?f?Ét?gsµ×zd4FGL J1514.6-2044¿ïÒ÷ޜ"ý@>å.rÚ0À:uÜ£¥§À<Ný&g@ìF±ë@ ¿þˆ1?Ã)Wɱ?³Ÿ™/Ò?ñ*¸¾«¢@25¯O>?ïÿŒÝÉtS¿ÝÀÆCÆ©G¿á$gRõpZ¿ãšÍv?ø¿ä;_‡O:¿â"«äøêAGNbcuPMN J1514-2043?ïþtBïI+?#%6ÿ/¼?(»ÑmL¼?#%6ÿ/c?ïý"T^®?L•i¶ÍL?4e]
‡Q?L•i¶ÍD?ïëºc°'ì?o¹	?dEœOn³?o¹	î¹g?ïÙ_MUå?\ê~D±SÃ?sP7ÙU
¤?\ê~D±S¹4FGL J1514.7-3617?îuMÒq/U@2)•þÚfÀ9ñâ,°b3À<ßMØÐç@1gIp@e›Ã?…Q?¹ì6Ÿþ8?Ï›À:m9@;òá3Œ@©›''3?ïàÏ6iI¿ÝóæÐ_~¿ã9 ²ýï¿æTF›œS¿êjáj)¿ïûÊYêWAGNbcu3FGL J1514.8-3623PMN J1514-3617?ë²X-"*?º¦èы?Á6ŸI³›V?º¦èы?ïÚ™M¶.?'«áWî‹ ?rÀ3Y$é\?'«áWî‹ ?äŽÕí
?·"²ž³i)?ÖâUÊ%ëÍ?·"²ž³i)?îÏDGeðK?†Æw½"*\?£»‰ û4?†Æw½"*\4FGL J1514.8-4748?íÑ]'Tœâ@ Ü˞Ïc€À8ñOäCá×À;y´{/P@ÔT¥sÂo@M/ãóYÿ?­á©þ–žh?º">eìC
@
~BZîc @xŽëád?Ýw€À政â,'à°«¿äS0¿äÕð'3¡m¿èÄ]'"ƒ¹¿ç ¿B Ž€AGNfsrq3FGL J1514.5-4750PMN J1514-4748?ïæ§z-²?j%_"ŒØï?iãX…ÒMu?j%_"ŒØò?ïìßƓÀm?{÷®)¯¹W?c 9l?'W?{÷®)¯¹Z?ïQŒm5²?Ž[p¤'Í9?•ÎlRYI½?Ž[p¤'Í2?ï²µU¶¥a?i~†buÀ ?ƒRª'V§_?i~†buÀ¤4FGL J1514.8-0949?è*ßîáÂ@C¢õ˜ñÀ8äŸM7ÁÀ;;Ò\XÆk@RgÈOƒ@aC?º"ÄÐÿâN?Ä?ðEwÙU@(»ÆKç@ƒá…Ói¿é¥Ï½—ûŠ¿äžæ.CŠ¿ã؎¡îÒ±¿ãÇÏ7
XI¿è˜Ï¤îar¿ê2ßP]¦AGNbcuPMN J1514-0948?ïÁƂ6þ?€>¼à´Þß?¾¿d€Æ?€>¼à´Þß?ïý/ȪßD?N/J'L‰'?6º©éB?N/J'L‰Ž?îC‰âúsz? ˆZÊöºò?«ÇaÐXÈV? ˆZÊöºñ?ïþ¿"%ô?›~è"?$Í ¾'ÿ?›~èƒì4FGL J1516.1+4351¿ïi.¤@L?ނ׶5À:ÉOµò–À<iàš	+"@É´¨"²z?üO§r 0?àxïÕæQ?ægë×TL?ý`« ªšs@…çë·¹¿ë~ê÷Z?¿äöHñá¿áº cÏ¿èΦ´4P¿ïÿšêÒqQ?ïú6È)¨AGNbll87GB 151444.4+440102?ïøùr§+±?SS)ÿ ²º?L5cQ;?SS)ÿ ²À?ïûÔ˝þ?[K«{—'?@¬Ñˆ°b?[K«{—'?îy=2Î?\Ôaˆ!w?®˜nÜ,Ó5?\Ôaˆ!z?ïç2CÞ_?aó¤…x©?hÍã¼!¢'?aó¤…x¬4FGL J1516.5+0015?Épxf~Ô2@G}$
=À:$í`Á
øÀ<6ðÊØÖÆ@ª4†O@ßöZdÐd?ÀFý•lŽI?²À´æ| b?ñ §". @ÄÓ6Hfv?ïÿÿÊPË¿ã»l‡è—.¿æ‡Í‰‹.¿êT
¾ÊÖ}¿è'vYùpš¿ïýHàÄ{pAGNrdgPKS 1514+00?ïø~™ô‰ð?U†IónÍV?N˜-ØB«?U†IónÍW?ïóŽ6Õþ)?p—4°°?Xã'T® ?p—4°±?ﶵsVèV?'wãÎ4‰•?'R£*EêZ?'wãÎ4‰"?ïFûáþß?€Î¸]k€?— ƒÝà$?€Î¸]k4FGL J1516.8+2918?š7Šè6@M©'Dé>À:Òwú øÀ<‡Ó*´ßp@ò_­Ád@¯œ'r^?¾` |È念Ëœ¡
ý?÷ÑÓíR~R@?¾VèD?ã	Ñäç¡¿ÝQò;_¿èÝ۝ ~¿âfÚ_\†ê¿ïátú}à?ïw¹_‡¤úAGNbllRGB J1516+293?ïÖ¾}yn¿?pû(z†÷?t ÁCH Ê?pû(z†ø?ïï­>y ?}èٛˆ=j?`RÁ†ßÿÖ?}èٛˆ=h?ï‡
°jÖ«?Š‹bX?Ž<"åJUH?Š‹bX
?ïœÏðaÅý?z_ؒ—?ˆÌ玀Ô?z_ؒ'4FGL J1516.8+3651¿ïíh"Ãô@Lñ¾ne8À;"ªLÀ<Ò6/fö@³B§'@
ª]6;ü?Ä˝bQý?·x°ëŶX?ì®Ö™íý@æ]êÁÕM?ÞU?bžÎ¿áåÓ)Þ ¿ÍU*˜ë¿êo¼árKL¿ßœ_Ý
\¥¿×¡CœŒéAGNbll3FGL J1516.7+3648MG2 J151646+3650?ïþ«z9öC?"uŒÝ'è?%H\`›æp?"uŒÝ'è¥?ïýw÷
?MU–vnÎJ?4@G߯ÄÇ?MU–vnÎ\?ïÒÀÐ!|?~ß,òǨ?vŸ—ïwBE?~ß,òÇ°?ïûü—jd?/BŠFJý?@
¢W'm?/BŠFK4FGL J1516.9+1934¿ïK`Ô8qs@Kð®Bž
BÀ:l3¹jðÀ<]úꉯ@HnÃ>Ú@WC³³÷?½êmœ™ì?oÌ]Ûþ?°¼0Gpó@q[$=÷Ý?ä³½œ®!¿×ö[üÕþû¿ëʝþ-B¿áâ™Ýâí¿âA&»×¿ïõ
8h&ZAGNbll3FGL J1516.9+1926PKS 1514+197?ïú4~p/?KKG±?G.?C¥ð?KKG¼?ïüޜpÙ#?P`d"H?9y6ùI?P`d"H?ï³cõµƒ?¯rÉ(œ?ƒ''º?¯rÉ(—?ïûè$?4اNQt?@_lE¹tV?4اNQc4FGL J1517.0+2639¿îâÙøRE@LÒÂ&€IÀ:¦7åI›UÀ<éᰉ @fâæi«ë@ü¨"1¡?Àæ'w2?˜hͧpÐU?×ւN8ó@«Çæ2)¿çsø`îW¿ÙJzAå}ž¿èxDµ;·¿Øñ±ž6ó¿åTˆM@ûs¿ðAGNbcu3FGL J1517.0+2637SDSS J151702.59+263858.7?ïþˆuJ?#™ÖKj<2?'x®«VþÉ?#™ÖKj<‰?ïý^9y¬é?P@²»3b?542˜¼a?P@²»3j?ïì7wwì'?h¦©^k¡¯?cȈˆُ?h¦©^k¡ª?ïö oi?Eãª#8K?S¿ÓÅ!-P?Eãª#8.4FGL J1517.3+6630¿ïA &žžZ@FZý›¡²À;BŸÿå(
À<ÏèYmZ@̘×ÒºM?ÿJBÉ©+Þ?ÙÚ €a?Úڐڮ6à@u4½vît@^ðù²?âÊ¡¿,ü
?ê{|½ë³m¿ãøÄL0Z¿ç·¡Aƒ­õ¿ïþÁU F¿ìÿ8?®ŠAGNbcu87GB 151628.7+663843?ïìÀƒ[þ?i¨ÕÞ#"?c?ê|¤?i¨ÕÞ#!?ïôÓN|^Í?mvàü!N?VYcBeæ?mvàü!P?îl#þ;À?˜'…#B®?©>-ÀCô?˜'…#B°?ïȗدh?ˆ!ìöLU?œ¦íêØ?ˆ!ìöLU4FGL J1517.7-2422?Ç%…'¥&‹@;"ŸDÔEgÀ7o¡vݬïÀ;$óMj@ËBÎܜy@¢U°5½Q?")A9R©h?#59GÊD@À"<jêZ@eŸ±aâ?™—ÿ)‰¿ßGà~ÛRL¿âÛ­p3T¿à¾Q	¿¿äæ
`:Ó;¿à˜ÖšíWAGNbll3FGL J1517.6-2422AP Librae?ïúN€ò?EÀN+hœ«?FÅÿ¿¼5œ?EÀN+hœ©?ïúE9ed~?^6­e ߂?Fëjn?^6­e ߊ?ï½Ý̊×?"ä!)ž%æ?€ˆŒÝ{Ê??"ä!)ž%á?ïôh"@
í?IòŸ.–Ë?W.×ê&t?IòŸ.–²4FGL J1517.7+6525¿Å§¬ÃKñ@F²-VÀ9e§Vñ~À<-s?'½@ ®F#û³?û¹9±Êé?«þDZF?°ìȀ6ò@àäJ7\@	ãÔùl"?ïЬU^f¿Ôœˆ Þ¿á,V4¿û-¿Ððú¾øxÍ¿ØlD̸«¿á$¬ó±³AGNbll3FGL J1517.6+65241H 1515+660?ïþTFø"?%¡MõL?/J»v¼º?%¡MõKÍ?ïøÊjÌ}?`q-îÓJ?LׂTÎP?`q-îÓL?ïìz®Ž¦I?g´Å"zm?c…QqY¶³?g´Å"zq?ïŸòá²?nÝÖ,®83?ˆ~G»S¹?nÝÖ,®834FGL J1518.0-2731?éì©OIü@8ü*í"1À8×äŠX³öÀ;ÐÞô@ï_íüGd@E^ÿiØ?§¤yá1L˜?'ô;X¬Ñ?ê?Q"W6@©¹qPON¿"Òæí4v¿ÉŸ0²Os¿âVæáËâl¿Üýð;ø ¿ãRÄþ¢1ï¿Ý%[[ÕAGNbll3FGL J1518.0-2732TXS 1515-273?ïûÀ""™Ó?<øÂéùuÙ?@ÿwu˜µå?<øÂéùuÜ?ïýö>¶wÖ?FæI璡?0N
LAP¹?FæI璡?ïëPSD'É?pRÈØåW?d¯¬»}7;?pRÈØåS?ïý"¶þB¥?+9Dª6?6êH
êÒ?+9D©Ý4FGL J1518.4+0750¿Â}Oƒê±@Iãø¶À;¥Š6OGfÀ<϶4ÚÓ @!æ©ÎÅöD?øFc[ïêß?ჲ<'Î{?Ñ[Þ£ˆ?ø@¢òÞ¯M?ÿ8n±d¿ï«¨Å†‡n?Öo'nÚ©.?ïኔC"¿À"¢Êšî¿Æ%
€œ¬¿é5<ø®ÒçAGNbcuNVSS J151826+075219?ïò'ë¤y?X*àÑV ?[°)ø·4?X*àÑV¤?ïû29†'?[å@E|H?C7‰å¼¾?[å@E|K?ï²*J=¿Ø?€ú-~'è?ƒump	ì?€ú-~'é?臭)®?p¸YTŒÚ?~«1þk)´?p¸YTŒÖ4FGL J1518.6+0614¿ê¥á½Úï@H¥Ç%ÃÞèÀ;NÉ&O"À<¤À²W&@!¶¿•×˜?û·Š*ÍB?È8uý³¦?")ê4;ÆÖ?ÑÁ߇Oj?ýÓ*U"¿ïðrXâð%?ïÿýfG³¿ä·K%˜?ý¿È¾ð€±a¿â›ëþì.½¿¶W¦Úõ¯oAGNrdgTXS 1516+064?ïþÇßþì?Æ·›v|?#'à<O?Æ·›v|?ïø²Zì?pA¾é¯?M6—ÇìP9?pA¾é±?ïïϊÏ?f|<1§÷Ç?`rû0u0ß?f|<1§÷Ã?ï³2?ò¾B?s–
Çj`T?ƒ3pPoH?s–
Çj`U4FGL J1518.6+4044¿æ[kÉDð@Lp'À‡D,À:¢"O…yQÀ<¡ã¼Ó[@ *4~6çž?üÕnvÖ 3?½ãpþöÌ?¶Fçeç¢?ú£é~´;@èîݘÌë¿ïýI׺f™?ïúþ§°´¿ÆS&ƒ!ˆ¿ÜèV*¯3¿ßìÑ$o¿Ù<ƒÿS‡¼AGNbllGB6 J1518+4045?ïùþðZE?J
7Éw4A?H?®–ë{?J
7Éw4C?ïóÍë³Å?p—à£'•?Xd(˜uñô?p—à£'"?ïÝý¥Z?sõ"%/?q@-~R¯?sõ"%/?ïs¼H0?‰M;5ËC?ŸQˆvùüË?‰M;5ËB4FGL J1520.0-0905?Û¬N½W@CwÏÃøõÀ:ÌØU—À<W÷øʁ™@ Ú³€ ?ÿ'º¤ê?ÇX›w•7à?Šû«Uè?Å™bg(@«"ÚJŽÄ¿ïÐ/",z²?>·Ë´¿åÄCá× 
¿ØóY^@'7¿é§Û?×$¿'aAGNbcu1RXS J151959.7-090434?ïíàN£?^×4… nÑ?bý±í]?^×4… nÝ?ïü.èÂ?RpQhvDY?>ˆ¿Ùì?RpQhvD^?ï–þUˆC
?ˆx¸©À¯à?Š@jï=?ˆx¸©À¯Û?ï—0¹¬­?øþÊ+?Š3ѼÔÔÓ?øþÊ'4FGL J1520.4+5546¿åäÎd§'u@Ilë¯#À:‹F¦­~SÀ<ÇúȈšn@29¹µú@'DEª.<?ºªlЍ̇?¥1B#Ÿ?çͬ[==x@²çôE¿ç£¥€š¿Ü	»€Hj¿ä­ÂC±Ü¿àAöD•[F¿æ ß=Ù¿é§E‰w§AGNbll3FGL J1521.1+5543SDSS J152034.98+554256.9?ïò¹'YìÆ?TU[–?ZŒÛL&t£?TU[™?ïû |'ˆa?V΄eáëw?A~aÞw…?V΄eáëu?ïÕ¿KfR?€Áš÷]‰?u ZxLÖÕ?€Áš÷]ˆ?ïνÔ¶\?eÃ5šZk[?x¡þ$Ò=?eÃ5šZkV4FGL J1520.5+4209?ïÿýç¹B@L÷< À:——sN¬5À<•B›†ä@]"s퍍@*½Bì?ÄûÆnäº?ÄúÒB¬?ùé˜dæ3¦@³ÖwñS?¿·ø·otØ¿è•*™1¿äö3kgW¿éÞá¢Fç¿è_Jþ«í¿ðAGNfsrq3FGL J1520.3+4209B3 1518+423?ïƆHµ?´3'4ÈË?|¼ðÛö¥ô?´3'4ÈË?ïüޞ@??P|¯Øš?9•ýü³?P|¯Øš)?ï"焦;~?‡ßƒí峛?ŽÆÖq L?‡ßƒí峟?ïúÆÞµ–?2ê{ëՈ?Dä…)§¥Ö?2ê{ëՕ4FGL J1520.8-0348?ïýq—:|(@E@j]këáÀ9e¾¶‰"iÀ;ÇҝÇ%Ä@ ®ÏÑ?øÁi÷ë^ˆ?·5ëŸJÞ?Ȑ°|_!#@U¨¸ñ@zkði	.?ïéÐÒj›¿Ò±Ä}óË¿¿ÒƒÒ‡÷°¦¿Å"¨™Þ¿ßÞ¼¹YR'¿äܝàP7PAGNbll3FGL J1520.8-0348NVSS J152048-034850?æwñëx¡¹?ʉ0ãyº?Ó)¼Ž?ʉ0ãyº?ÙrÄiK?×Ñwœ!‰?ã~FýK[?×Ñwœ!ˆ?éäÑ@¶?±µfø·3?ËÏàlºý'?±µfø·3?ÕâJ®ÜU²?¸=#uDpÁ?åÚ¨'Õ(?¸=#uDpÁ4FGL J1521.1+0421?å­8TO"ô@GÖbýüÁÀ;<-šlþÀ<'ÐÛOF@¼ú%6ñ?þÝR¦–_?Ó+-€@Ø?Óµàaª@¡B‡N@:à\̉±?ç(-í¤?ïÿáÍì¿ÚÞ;õy"A¿âÄ»á˜
ù¿à¦ºŒ¥¿ïÿ€éŸkkAGNrdgPKS B1518+045?ïû27oU¢?Aö 'Sôƒ?C7"B©|G?Aö 'Sô}?ïùK'õØÄ?`a[ŠâV*?JÑô(œò£?`a[ŠâV0?ïfߘ}Å4?ŒõJc'?"$ðGY"?ŒõJc?ïQÉ9üÌ-?ƒaô2É2_?•ÆØÀfzU?ƒaô2É2_4FGL J1521.8+4338¿è)Ž¡õ	'@KÊÒ¡øã¬À:HÚgÀºÀ<P·»*ä@'fuªÑû@DEÅ.î?ÀÐd[õP?³FþÌX´?îÑÕJIÐ@#ö½8ÿ¤1óÿ&øN¿æÌuúX S¿ëÎÊϜ‹¿é^ÑF¯ú¿ïþÔ¡­dR¿ïÿøãúAGNfsrq3FGL J1521.8+4340B3 1520+437?ïþ²´lç?)Æԅ¹90?$Ô¹1'ã?)Æԅ¹9?ï÷z³_ÈN?q".»á?Q
™@oe®?q".»á?ïßŃ0²'?nÔº¤Xê?p>g¦·‡?nÔº¤Xõ?ïÎ,ukL´?j4¨hãF?xéÅJY¥¹?j4¨hãD4FGL J1522.1+3144?ïÙ0B
"@L'€uMÀ6¯ÐÈÚÐÀ;,âó¾ý@þH¸Uœj@õ¯¯…")?"}k,fˆ?²LDÀé§@&k9:´0õ@ ^œAk°¿Ð9wн¿â®L·2¿æŒï'zß¿æ»Ráú0ˆ¿éK·ž'QÒ¿ì]Ñó¹AGNfsrq3FGL J1522.1+3144B2 1520+31?ïð4fsjì?X >Jè›?_—3*(°?X >Jè›?ïËWüÊ#È?>lJð?zTšîÈ?>lJî?ïŒ>)¦ä"?ŠsÀvÏ?Œðu–Fލ?ŠsÀvÏ?ïxBÀÉ"?"ÏéT`i™?÷§æЙ?"ÏéT`i™4FGL J1522.6-2730?îœ_Îsí7@8fnü7£À8¯®çúÀ;"Ú")=@G'%\@·g2Ë?¦aPÒÖQ0?ÀBLUÄÍ@Ó:aû›@}*x#¨?ïJ?SÒåì¿Ý=E@¿áÆipÜáî¿âeÁ$øÞ¿égM·B÷Ì¿èŠS«x¿.AGNbll3FGL J1522.6-2730PKS 1519-273?ïÚ©ºnþ?s$P€I–?r«"õH€³?s$P€I"?ïç›(0~?{°Ã¿P߆?hd×Ïꁂ?{°Ã¿P߃?î­k˜©¶Ø?áYl/m?¥)Fud'"?áYl/p?ï_ڣŭ?|¶¢"¨?"«‡_ŠZ?|¶¢"ª4FGL J1523.2-3941?幞aħÂ@,Ï9ó@ÔÜÀ:š
s÷H¡À<&« ,ZÒ@/b™'Y@¥D]'""?҇BlA?یo¤þ|@‡XÅÉ£@ÃNú#"?åg' Ö9]¿×9PC9e§¿á¸n¦¦ÈV¿é*è¬&d¿ïD‹ûbâ?ê,Î?=­‹AGNbcuPMN J1523-3936?ç
DlŸD?ÆwçiÓÀ"?Ñåáw&Áy?ÆwçiÓÀ"?êCäe¡WË?˲G
yÅk?Æðniz Ô?˲G
yÅk?èÊZ8?³-âg‰ì?Ï£è֕‹!?³-âg‰í?ìIU*{ø*?¦Þmô: ?½µV¬ >¯?¦Þmô:!4FGL J1523.2+0533¿íEU©æ˜@GùÆøÀ;$1âÑÀ<Ô{¦j@ BE‡H´@3c¿Âù?ÅZÒ ãe?q4a†'»‡?¬·øX$Ú@ƒ&ûíKÈ?ﱋÈö~w¿çâ³¾ÞοäӅþÝD¿Ù­_H•p¿èQrÿ&`?ÁûÃ	€AGNbllNVSS J152312+053357?ïø2Qۘ?Iz÷K¸2y?O7²¸'¥?Iz÷K¸2t?ïû§Šþ7?nèÙMùÊ?AaÕø¹?nèÙMùÎ?ïà(QÓ?y«ÔØ'?o×®,üä¨?y«Ô؉?ïꈪ;Û²?S+Lè\?ewUÄ$N/?S+Lè`4FGL J1524.8-5904?Ý1Pxv¤¿ýªôj ‡ÊÀ90êþ;·À;û¼¤`@ü†x)²V@¿:I§ê?ÀM^7?³Ï1VT'?òá+^R›®@=ÂKIU?ïqéQgÑ ¿äÜ-'€wŠ¿å'/ò?M¿à@RÖfª¿äÇnôªah¿íV ö…-AGNbcu3FGL J1525.2-5905PMN J1524-5903?ïî0?"é?cþÌ¢&?aÏÀé{?cþÌ¢?ïùƒqy…l?jEsXè5Ì?Iò:êH¯?jEsXè5Ë?ï:H|>É?•Ødl>XÜ?˜¶ðx?fë?•Ødl>XÜ?ïSÓR¨/Ó?N(ô'qñ?•…•ªúh?N(ô'qñ4FGL J1526.1-0831¿ï·ôä$1@C$Å~#òNÀ:d'>2j¶À<UW1?=-@ ÞÙꗎ?üèÀ˜áãµ?ÄÔ~\|W¿?ÈaZ8Ô%@2_¦XĽ@(jž"dÿ¿ïí¿‹›ª?ïøÒ¿€#¿ÙHÝòd¿Ø¸ƒ¿'¨¿ê Æê4¼ ¿Ã%I:±ÃAGNbll3FGL J1525.8-0834GALEXASC J152603.17-083146.0?ïáÖÓµVu?p€wèm€?n),J©Š{?p€wèm}?ïöÇo"Ú?hiÙ~!-ö?Rq!æØLˆ?hiÙ~!-ö?íÙOÒìoP?¢Y͸'ðÈ?±5hœ…{?¢Y͸'ðÇ?ï!÷7b?‹ Gäå?›Ý¡"±?‹ Gäæ4FGL J1526.7-1529¿íÂ)ž­‡@@J#9ÀìÀ:¬ðéÇ´À<f]ú‡;@ |o»Ï¤n?þaÝ4ùÜÐ?ÆV©Zý?¼Ùz°m?öŠ"é9?ýÿrêg¹¿í$

[³?ï鯁7x¿ÐÀ¸âŠ#Z¿á},±8ò¿à	gB…œ¿âçsâOëÑAGNbcu2MASX J15264667-1530269?ïúAÿ˾?CŽ¤Ýä'Ø?FøÑà ?CŽ¤Ýä'Þ?ïí_rÿH?uõAd=K?b á¸¯?uõAd=N?ïÜiYÐhÕ?vҏ
"Ìs?qËS˕ƒ?vҏ
"Ìk?íñàæ%?˜Ì
ý–'?°wˆøÏöÎ?˜Ì
ý–'4FGL J1527.3+3117?ætòr+@Kò`ÐÕÀ: w!ŸŒùÀ;ù"GÁ`@Á¾V<"@;`äFf?Æ? fÒÇ俯ÈԀÜo"?à¡…÷%@÷§f‹Ð-?î†'_8u¿ëIé7'¾¿à§û\,Q¿ì#ã@Òٿłìƒ÷Eò¿ïÿ÷fÔJpAGNfsrqB2 1525+31?ïüÉH<%!?:L¢oU¹?9µ¾ÖõŽ?:L¢oU¶?ïýXÉÁ«¤?P9Ô¿Ë?59±ò¢ây?P9Ô¿Ò?請'Ÿs?ƒ	OnO?…Q›˜#.?ƒ	OnT?ïöd	AD?GoPði?S7ìá}v†?GoPðK4FGL J1528.2-2905?î8ש¢j]@6d)¿*åÀ;(9Úí!À<Rӓk@ aOƒöÅ@ž¡%Š?Ç{¹ßµ1Ñ?"'Ë´êz?ÀBE_Z®w@kÈíºX?ïo×ÿ/öh¿ç¥8ž¬þÑ¿Ô܋ò)ô¿ç…L»Q¿Ï¿'ýs2Ó¿çV¯¤ÙšAGNbcu3FGL J1528.1-2904PMN J1528-2858?ï÷ö¡Ñ?Rž)ÖÇóÊ?QÅÀ¼_N?Rž)ÖÇóÁ?ïüŒªwàê?[P§‰CW?;š¬@ø«–?[P§‰CW)?ïÎDkz?`?|Š´ñËĪ?xÝÊBàP&?|Š´ñËĞ?ïÕÅärwÌ?cS£1V¸?u
Æļ?cS£1V¶4FGL J1528.5-2240?± ¥à/Û@;bÏÃøÀ;7šr­™À<¨©Û0=@ÄøqÁ8o?þ#¨FÇ?Ԁ#[¤Ák?äê<ŸB¥í@SÒz‹·Y?ùQµ)mÇ¿ïÿû˜'2?ïÿjÕþпÂÒ練'8¿êRz᝔P¿ç"Ü0¿ïÿ(3û°AGNbcu3FGL J1528.7-2247NVSS J152834-223522?ïäÁ¦w?
÷ÊT•?lGË1L?
÷ÊT"?爼"æM{?Ñ4Ú¬ÃR?Ðî†Ö3e	?Ñ4Ú¬ÃR?é1¼%Ê?®ÓŸ†¶³
?Ë9k"×ç?®ÓŸ†¶³
?ÙpT&ÓÏÈ?µ4µOxbl?ãGÕì–?µ4µOxbl4FGL J1529.2+3812?Ù¾¢×Dd@K¤÷<ÉÀ;ŽõѨÕÀ<Ò¨Rcz@^{/v:D?ÿ͕I¨À?Ég=üºÑ"?ÁEûø3'ä?ø"¸vÔr³@Ë܌ÞJ¿ïÿæ¦Sf?ïýWÿ›V2¿æ3߀ƒž¿Ú
˜à66¿ÝÒ	L¯Ûû¿ïÿûbâMhAGNbllNVSS J152913+381217?ïüUÌ{Ÿ?A}!ÙHh?=Qœ#'E?A}!ÙHq?ïòy<Oâ\?qs(~O…Í?[
‡`;JÐ?qs(~O…Ñ?ïŐÙHé>?ÄØ{IÁ[?}7"[‹a€?ÄØ{IÁa?ïBO
*ú?ƒ†Y‡ñ¸?—¶Z¿ ©?ƒ†Y‡ñ¸4FGL J1529.7+6733¿ï]>ùwÜ2@E 'RTaÀ:ø+ìïÀ<Ú]^è@#f½ú!@ÕÓ;{×?Ä:Ôd¬R?³En߆¸Á?îï–ü0g§@•ÀR@Á¿ïâwú ø?ï5Y³Ð|…¿æíUj• ¿ãËЮٝ¿ßÞÖd¦à¿ïÿ€ß֕AGNbcu3FGL J1529.5+6733WN B1529+6741?ïü"3à'Â?:œ£ßa|?;Þ`ûqñ²?:œ£ßaÁ?ïý''0L?T›îÖÿ?6Çóî}•?T›îÖ?ïÃL†´Å²?}ÛLÐ	.?~Y¼¥'?}ÛLÐ	#?ïã'|"?_R'Oë?l}ƒý{ýŒ?_R'Oë4FGL J1530.5-3026?ï¹(Ùn2@5öè)I¥À:"¡°¿P
À<IŠÃ=@ Ûà­T@š¶ÐF?Æì,c‹?º?Á¶Ašÿö?ý,…]T@˜%Ùç½?îåA7Ø´b?áuD C¿ÞA&¦\ö{¿ÛìVÀVë¿äUÜär¿ïÿséèwAGNbcuNVSS J153041-302559?ïï™æۅ?bÀ¥ë<ò?`øf${©?bÀ¥ë<ó?ïݏˆÅÿö?Ž'ö+×ìk?q8;?Ž'ö+×ìk?ïÈ#/òÙ?|"ò)w?{î7è"1?|"ò)w
?î­RMõ¨?KSæÕ?¥*Û ¯¥x?KSæÕ4FGL J1530.9+5736¿ìL©€Y=@HUŸ<pɗÀ:¸Òñ±‰À<̋Ջ¸0@$֐šíW@8‹aÈqô?½+¶g/º?ž.–¸¶ã?âTæA?ýS$Z'hÐ?ï bb ´¿ä	£ý˝M¿Þ†\㔏¿äí·(Ùº¿É$û(Õ·¿ä+4̐fëAGNbll3FGL J1531.0+5737WN B1529+5746?ïï
Ù}m8?Y>
•³¥?`ò&''Èc?Y>
•³¥?ïú0E¬Ï?\~S	Ù®?G>ëéLÁ?\~S	Ù½?ïÕ'»µï÷?z¹g W6g?ul"%r?z¹g W6g?ï†'ßQ?}6tG»un?Žv8¹ë½?}6tG»uo4FGL J1531.7+4710?à0w'ùø@JpÄÑ¢À;:›!YÀ<çK,N<¤@dªrÚ½ü@ƚƒ¤dÏ?Ä[}i¸*~¿—ïY¥ÉäÌ?ÔsæÂer?ó݋s¼e?ïf[~«Ø¿ìB¾$=w¿»òRÃFfA¿ãŽc¥ÁÆ	¿â?~e`¬é¿ÓS'úð̆AGNbll3FGL J1531.8+4704SDSS J153139.78+470705.9?ïñJ½Ø%?^Ùî
jÃ?]j"Oµá²?^Ùî
jÆ?ïÊÁ"?U?ŒMu2$¬œ?zŸ6`Uqb?ŒMu2$¬œ?ïÕ~vgn~?yÒQÄPi?u@ÄÌHÀ'?yÒQÄP_?㋝?'¯O¿,û·?§×1ÇFF?'¯O¿,û·4FGL J1532.0+3016¿éqŽ–·½²@Kh'£"¯À:ܵxqÀ<\…íë*†@ÐÒ=úâ_?þHH¦4?µ¦â­^Èb?šrFQэ?ä‹Lš† @	'öWµžˆ¿ã¬,ÿ<‹¢¿Õ¢Ô€ËA‡¿à=Œó˜ép¿×®Ué@ Ú¿ãyˆíyë~¿ÝÑLcZî8AGNbll3FGL J1532.0+3018RX J1531.9+3016?ïþ[Cxh?!ÙèmmŒ?*KÈ~	??!ÙèmmŠ?ïü)boȺ?SX_"?>´ìº3Í?SX_"?ïø·§'Ò?Y¦¡Ë¬5²?Oñ!a´¸`?Y¦¡Ë¬5?ïõK<è<?DOÝæ%?Ui†/ñˆ7?DOÝæ*4FGL J1532.7-1319?¦ñÁ@@Û$Aþ¨À7éï®y$¯À;iTJ0@½†QŒ@‰~Ü~ñx?›D§¤Ê$Q?º(žYÇÇ@{•"d~@€6ŹÞ?Ú¡½àåοÜü""+É2¿âc[Ÿc6¿å
î \+z¿åTw·¿èÖÍÏ2ÙAGNbcu3FGL J1532.7-1319TXS 1530-131?ï찁æÈ?c6>ªá?cçO~8'?c6>ªà?ïë­b%÷&?€ƒs"i¡Ç?dRÚÚW?€ƒs"i¡Æ?ïn_³•?Õ^‡É4(?'<"	`?Õ^‡É4+?ïû¶æ¡?6"kj6e?C'$gé©?6"kj6)4FGL J1533.2+1855¿âY‰fTæÞ@JóFí$À:Y-2h2À<Y´E‹@ ú$…ñF)?ý
fóT?¸CÀ°E¿–¹Æ_ËA²?à'ß@lך?ò,{Þó•ä?î_8	[ÉT¿ä3"âz´¿àù&ÝdtŸ¿Ý…¥;8eL¿Û¢†\ûـ?•_m"îžAGNbll3FGL J1533.2+1852RX J1533.1+1854?ïôç&Rڈ?SWû¢¬þ?V1³ZJíþ?SWû¢¬ë?ïBƃ·ˆ°?°ý¦&BZë?—§/‰ê?°ý¦&BZì?ï×J<-?|nWÖ	?tZáýðê?|nWÖ?ìkJòõa¡?£Ô}ÌNq?¼¥¨hTò÷?£Ô}ÌNq4FGL J1533.2+3416¿ÐI°^¬@K\
è³³À:4nµÀ@ÍÀ<tݒîY@úŽñt÷Ï?üo[Ømë?¾Q™Ð¡?»Ê³íض?ÿwÑȵ@ǙÚ\,|?ïö&' ®·¿àׇB_ ¿Þåqúfä¿ÆcGãnyÛ¿æ+iÀú)¿Ù=Ÿ¤u–AGNbll3FGL J1533.5+3416RX J1533.3+3416?ïüð V£?>b¥›¦G??hzýJâ?>b¥›¦\?ïøÈ'É7#?a¥CO-«?Lß`Û#rB?a¥CO-«?ïìÜ)³HÝ?jš¤:ۓw?c#ÖL·"—?jš¤:ۓ†?ïXÎV§?w£É!À8Ê?"æ5=kí?w£É!À8Ê4FGL J1534.8+3716¿ï|Ç(›i&@K"^þ"vÀ:†®û*®)À<{¦_z¹Û@ -¤f&O @h	¹½%?Á…dXo,ß?tWíÞ²€Û?¨üð-¢P@®?aê«°¿ïþöë"Gù?ïû³ÀsQ¿çác'Å>¿ÚT°ÜVW¦¿ßaÿÏ¿Ü3oce*&AGNbll3FGL J1535.0+3721RGB J1534+372?ïþ›7õzÞ?!–>L8?&L€¨Rš?!–>L4?ïýLxÿ1?PÉ¿»ˆfS?5œ8ž#?PÉ¿»ˆfO?ïóJ$+ÚÌ?`²BÚ°O	?Yk·¨Jg~?`²BÚ°O
?ïôcÒ.<K?LÎaììÇ?W8[£‡l±?LÎaììÂ4FGL J1534.8+0131?ìq½\`@Ev¼ÿ À9‰èK®TÀ<½ÅÈ̍@ÆÑÄÙ8k@-ú¡ò-¯?©ã,›Ð'º?¡‡ê<ÒG?ó-ø–2æ@:ñž"S"¿Ì¦bÀi'¿ä­ºþ™"¦¿æRÎÙíFÀ¿åù?¼ ¿æneÆ-¿àËVq_iAGNfsrq3FGL J1534.5+0128PKS 1532+01?ïþ¹¤'t?#å~TÈ)?.Äe½ˆÍ.?#å~TÇb?ïüŠ@çn‡?PCXE6
?;­øċ¹ô?PCXE5ö?ïéÍOO?gÞª½«s?f2°ô°ç…?gÞª½«a?ïÿƀûß>òÁHæÒ»>ü¿'qÑ>òÁHæÑ4FGL J1535.0+5320¿ë[W(^Ãü@I;:h²À:ÙUvT4À<»×¿o8@ ¥D#ñL?ú¿Ãvâµ?Æ»ª¦ds?ºs欜֐?ôŽ¯«SÖA?ú3–b'$¿çª=UËä¿âvþèÓ¿¿ãOb2Ôi¿³à}:"¿ãc܉ٿÏ%ï¨ÄÚ»AGNbll3FGL J1534.4+53231ES 1533+535?ïþ'H®¸ ?'æ'ûÔD"?-‹uuì£?'æ'ûÔD­?ïö³Æp^¨?gÉ#¦©+?R˜sB±{?gÉ#¦©+?ïðZT*ý?oÒ½¶Mè@?_KWéª-?oÒ½¶Mè-?ïh\ª3Žÿ?}Î iB	?'ôj¹Ž '?}Î iB	4FGL J1535.3-3135?ïý­¾k[¡@3z'Ä"BhÀ;IØ›ïµÀ<"ü4µê@!¸îžƒ¹?üÁÃiv¼?ÔKí~ÉÈ?ÈIW·Ìàn?÷:Y²ù¼ð@¤Ç¦È+R?ïʺŸ¹¿îegÞ`ú?Ö»&F»¦4¿ÉÌWÇg2>¿æåöŸ..¿"ì Çm3×AGNbcu2MASS J15352963-3133461?ïÿ¬>¾j'?
?Whëç±?ðPe[.œ?
?Whëè
?ïû€ƒTO
?^YRõåÝy?Aýò®ÃԂ?^YRõå݂?ïÝñ i??v]J4"Ï,?qoËs`0?v]J4"Ï+?ïç&¨¯´?XÝKõwèÔ?hÙWoPJ7?XÝKõwèÓ4FGL J1535.4+3919?ì5¥Mí[>@Jøââ¸Ç\À:ÎNCYòÀ<½'_Á0·@–À©ÓÎ@çÚaàŨ?Ã#¤õÃ;)?ÅÃ[Ÿc6@S,ÀRk@m‹¿ï‰«zl­¨?ïý_Üßiˆ¿ÝsÃüČ7¿æ¼þùoÿçdÂW(¿Ú¬‡]ðAGNbll3FGL J1535.7+3920RX J1535.4+3922?ïÌ þN
?‡Hxz"¿?yïõØùK?‡Hxz"¾?ïñ9ò—Eè?uj'£Ë¯e?]ŒÑt1ã?uj'£Ë¯g?ïE²¤þ?"ò¨ðó¸?œ^I«`Q?"ò¨ðó»?îߛÚzƒ?Ïà²?¢OXWÂ?Ïà²4FGL J1535.8-4730¿í¾i"@Ô
ª}íÀ9òż7SSÀ;YË0ëZW@ÙQj€Ò@'þ?5Ÿõ?ʌ×ÿ°ÏÁ?ºŸlÂK¥?ñï_˜@Ê.¿çk(¢¶xÍ¿á­|5Om¿é
߆ã´p¿åd±û.·¿ïývƒ?Ñyé{VwAGNbcuPMN J1535-4730?ïü¢…Íê]?@Qîߓq?:ëѐ­?@Qîߓa?ï×(¦ù)?•´*" 7?tkû¬ƒkY?•´*" 7?î­¶¤…ø?œ¤2Ӊ?¥$•¿Ç ?œ¤2Ӎ?ïÊ|Õ°îÒ?n›Çr?zÁ•'ˆ—Z?n›Çg4FGL J1536.8-3155?ïþmÔ¶@3…7âÅ]À:˜0òçÉÀ<MãÕ'b@éÿð:»@nÅý0B?Å ¦ÿÝo?»17°pu´?ù»aj~#@ý«Ï§º?æ§,ßÜôã?îŒðÿ1#¿ê¼'ÂåÃ>¿Ëùt`$-¿èû,=WN¿àm­'"ªAGNbllPKS 1533-317?ïëèܕ«!?fjÙ+Xœ·?d#jTÝß?fjÙ+Xœ¶?ïî~F¡²?|Yýš™,?aá¹^N¬?|Yýš™.?ïLJƒáà?'ŸˆpSÂì?–v¯ƒÃÿÙ?'ŸˆpSÂì?ïö5ÀCí?{n«ò6µ?‹Ârï¤?{n«ò6²4FGL J1537.7-7957¿àNu]~À3rŸb0wÀ9wJ‡ãŽ°À<þ–µº@Cƒbu–@Òâu«}È?±	]Ýçãe?›Z*‡¬Ëê?é´/JWè@'ntҺͿÆzðv g¿âCF;M³è¿å¦ÃMÈ	ï¿Þ5|c¨Ç¿ç»ÿTßUf¿Ùa¶ÔAGNbcu3FGL J1537.8-8000PMN J1537-7958?ïûa)‰
°?:dc»ë;¹?B{YÛÉ="?:dc»ë;·?ïþ¿÷Ü?Kù¼4s?/ä'G?Kù¼4g?ïòˌ}µ?_àó&¥[]?Zhç•óZ?_àó&¥[=?ïõ¿"th¨?C¤gˆÔ†p?T€÷.­á?C¤gˆÔ†l4FGL J1537.9-1344?à˜"Lèó˜@@EæšÔ,=À;ý>" À<u¡gÄ4x@!ë¨îv?Í?ù6 hUSï?Ïô	Q¸Yx?ÌfÜX$­@WƐr©@ùìðٜi¿ïÿøsCÄ{?ï˜b'p?ïß°Ÿoœp¿¨îi t)¿äŽ¸Ê·H׿…ž:J…AGNbcu1RXS J153757.1-134334?ïû"#I´W??qu4ì©?A¯rÙ.ž
??qu4ìè?ïûn3Ò^r?]}Ó¨±W?BG0¶†7ä?]}Ó¨±_?ïϵ	"¥L?t³®h½ÝR?x%{=­Z?t³®h½ÝW?ï§N"[À?zÒ?þ`|?†,[;i
?zÒ?þ`4FGL J1539.6+2743?ï·Rñ#k@Jnž²gÇÀ9‡tw¡!MÀ<^c˜UÌ»@c"çQ@…¨¸ñ?®ŒÕ;d™?ŽÐ¸rwÂ?Û@ï~¨|‹@Œ+.,
O¿Ý UàÝ%
¿á±ˆmø+¿åc(>«	¿ã(c@Â	¿èQ¥^ɹó¿Úñ VL<ïAGNfsrq3FGL J1539.5+2746MG2 J153938+2744?ïþ g$a?("œe?.åùº
¿?("œes?ïüÕ§[ùv?S5_]¾Ðï?9RÅ 4KW?S5_]¾Ðô?ïìäæG1?a1©Ýè??c÷¸ÎÛ?a1©Ýè??ïÿÐmQÎQ>ï›çŠzH>÷ÉWÖ´L>ï›çŠzD‹4FGL J1539.7-1127¿ïˆ3tEe@@ëˆe"¯OÀ:!4–àµÀ<"ý2Æ%ê@ çTWÆ™?ü¨Ö¸ÞÙ??¾KÞ'ñ?¯|©,?ñ¥×Ë-\@œ‡VKJ¿îê´^–ä3?×p6~—4º¿Ó3ƒ$¸:¿Üã'ìý¿Ýt ƒƒ,ƿفí`@1žAGNbll3FGL J1539.8-1128PMN J1539-1128?ïÃ'26§?¥¦Sqq?~luæä¬]?¥¦Sqq?ïùýÿ6E@?c!j+úœC?H&êý??c!j+úœ@?ï¾=z€?™,Ñ"ž?€pŸ¿a`?™,Ñ"¢?ïtÈã©ê?~04¯%Ö?'fÿ£ŠÂ¾?~04¯%×4FGL J1539.9+4220?á'®`;@JTøœ^oøÀ:ñ/!U»À<·Ö™Õ(¼@BÉ0`@ÞKÊÙ­†?Ín
å÷R?Ò¹·FRË@Ü$Ts@ž‰XöU?ïú	Iú¿àì5]YøD¿åÑ,½ùf¿ãVq_i¿ì˜FÉ))¿ïÿ韖]ÐAGNbll87GB 153741.6+422719?ï³Ú¥:xÍ?'Öòi5æ?ƒ	V±aÌ	?'Öòi5æ?﬈ä@¢?":Ÿ]]t±?"ÝÆï×xÇ?":Ÿ]]t°?ìïZטÂh?¤Uýj¶O?¸…)C9ì¿?¤Uýj¶O?í©¨:Á?›F罅PP?·J³ò¾)þ?›F罅PQ4FGL J1540.1+8155¿ïŸÈ6U;@@{w¯d:À9 *aÓY¯À<ýÎÍX
@  óS
?øÑäcÂG8?±Ò-÷ `?µk½AX@>J`vb]?ÿØ&,dŒò?ïÿµøtñD?¼(ŠbÄñ6¿Ûh1AÁkp¿Ê.ÇΏ¿ÚØ4¿¥F÷¿Ðžñ;º–AGNbll3FGL J1540.1+81551ES 1544+820?ïëׄ|ó?fA>΄·Ë?d({âƒ(?fA>΄·Ë?ï,	'ÃÇe?³VšZ–Ë?š~ÍLJx?³VšZ–Ê?îëêÂÃóÊ?–kBTDv?¡ASÓÀÃ_?–kBTDv?쟅¹–? v‹?Ù?¿Ò7KE? v‹?Ù4FGL J1540.4+6606?ìXˆú­a@E'8\gàÀ;	j²VÀ<'$»¡+^@,B(C–@§£áñø?Åӛˆ‡"Ÿ¿'êŸÛۑ?ÈüCŠOO@¾¦y&¥¿ã3ßá& ÿ¿âHA'O ¿êgÖX€u¿×^ä|káP¿ïÿk»9ýR¿äFù^PBcAGNbcuCRATES J1540+6605?ïøÄ•Å?UGql*r­?OŒï¹¨íÁ?UGql*r¡?ïù]}탸?og"7FC˜?JŠIñ«?og"7FC˜?ïÎ÷F˜Çá?{¸îÁÙ?x"\³œê?{¸îÁÛ?ïðG ô/7?Q¥A­`?_q¾¡'t?Q¥A­U4FGL J1540.7+1449?æÄI䝞Û@Hiˆ;£D=À:EÖL¨O?À<XÑӜʧ@äA:2@57¹«?·`éàêø¿¤$QÛ¦?×e;$C@úV6mzW?ïýÜ9QZf¿æýé¥K¿ä½`t#"¿ÞÉ«…)u¿á¾ÁqN÷µ¿é¨ü¾W7AGNbll3FGL J1540.8+14494C +14.60?ïüþIm?BWU^˜]F??À
³¤€?BWU^˜]<?ïý^!F«o?L µi"ª?5õʤ•&?L µi"©õ?ïô»¸å™¾?g՛¤Ð€)?VˆŽ4̃×?g՛¤Ð€3?ïÜ"6b¯ö?[62*uC@?qîäΨ°?[62*uCE4FGL J1541.7+1413?ÁmK®Ô@H,ü'œýÒÀ:ψ[ƒ´À<€©={‹'@ Œ«hy7?ý|=¸ƒj?Ë6¢Êê?¼»HjýÏÏ?òÆ.jÑ@ÐØ;Y¿â¸J^Èã3?ïôhAÝÅî¿à@ÝݖI¿ÛÜ\AŸ\§¿Ý`½¨"¿ã6«ÃgÉ=AGNbll3FGL J1541.6+1414WISE J154150.09+141437.6?ïü†!j2[?9HÚñ¾šÑ?;Îô®m%·?9HÚñ¾š¤?ïú‡	Ä<?]¡2›"R?EãØïÁ?]¡2›"\?ïîä2Íå?gæ-li~Ã?aÍú2D?gæ-li~È?ïªæÓNå<?q=zÃÂ)?…FK,F°Ú?q=zÃÂ+4FGL J1541.9-2915¿íLnˆOì@4c†Â&€À:ŸBP©À<3bàŸèh@ h ¢¢V×?ýRÎ8ݗ?¹íY	[ža?¹+œïÑà@¼íƒüyc@°|OG'?ïæ'P¡Ù¿ÖWÀü_©¿Ë߬bôìÑ¿Ôè#ëA­¿âüæÛkÌ¿Ù78+>AGNbcuNVSS J154203-291509?ïðXår.?Z- u"üË?^ÅN5¤?Z- u"üÎ?ïÙw‡Ò6s?…½ñ.à?sD<äƕ?…½ñ.à?ïËÅ		è?}%Ps;'?zt{{è?}%Ps;…?îs¯.ùâ?‹"0òû¦Ë?¨Å
cÅÖ?‹"0òû¦Ë4FGL J1542.3+1801¿å^ÉÌd'@HÜ#|ÜÊqÀ:¦µ{wo£À<\š¨Rc@ù¦&oÖ@ ,ƒɖ?ËhO_8Ê¢?Ïÿâù´âJ?þ‹¾z#²@	Öv·Au@¿ãµ>p~]¿Ùãàd¯,¿èh‰ø;æ¿éç§^~:™¿îRËI?3¿ïÿ2FÄàAGNfsrqOR 167?ï᫵&?pª6'9ýR?nñTäJÚæ?pª6'9ýQ?ïør¨'$¸?n.ÔÝå`?N5_cm ÿ?n.ÔÝåf?îDnÀ?r?›F3xŽwY?«¿™üà?›F3xŽwZ?ï‹Úï'í?yßç‹çG
?	DÄô?yßç‹çG4FGL J1543.0+6130?Úyi†æ÷	@F°üø
Ã7À7‹g‰|$À;LãGb•!@ Ï6K?þdØâ"Äö?•#VØe˜?®vý@Ã@•B½ò%@
˜™êL¿¬"'È¿ÙK'àD£É¿ß´`¥_@¿Þ–ÖZ²Ô¿âÌdȵ2¿åcܺí§AGNbll3FGL J1542.9+6129GB6 J1542+6129?ïøoVZÿ?KyzåË
"?NB¦"ºg?KyzåË
«?ïìÌf'š?w[§Ûª?c3é™}gL?w[§Ûª?ïɗ¯¬CŽ?|Wþ92i?{4()Þ8Ä?|Wþ92k?ïê
×(%?TНÁ_.Ë?eò(×÷Ûÿ?TНÁ_.Î4FGL J1543.6+0452?î™Hô"Hn@E¯àŠï²«À9ð³!*3À<,œ \–Ú@ {ç_u0"?üxœ‰8#?¼W®'¥¹?²á°^­	Ž?ù(¤Ð.@
nòÿ'p*?à8Q_îýú¿è*<´¼4Ï¿áÄö¿w'¿Ô¤Vg®æ¿Ý˅å\»˜¿ßÚD.®AGNagn3FGL J1543.5+0451CGCG 050-083?ïþö¦iÛ?Ú+X‰Öm? ž¥™b=å?Ú+X‰Öl?ïüê.6+"?MŠ+Cr*?8®ŽN£`Ž?MŠ+Cr!?ï÷™â1-$?T®_›Aq"?PÌ;¥º?T®_›Aq?ïîþ®ä¤?Küè}˵?a=Q[ñ?Küè}˹4FGL J1544.3-0649?îÁ¢(»Nœ@BŸ¸gÀ9%'œüûiÀ;њ#,Tó@ 1ݘL¦?üðI ]?®ÎdÒg–g?«i¾_¡¦-?ÿAVâdå@Nn|4"?ïñâÀÿäý¿Ç=ÈwþiR¿ÙŸ¹Ù«¡¿Û R:µ]š¿àÔ7ŸÔq1¿ÔåÓc¿ÂùAGNbcuNVSS J154419-064913?ïÿ÷"®?ÃތD³µ?
œÊ,€?ÃތD²ø?ïüèx"i?L~š'ä¦Ò?8¼>ì³|K?L~š'ä¦Í?ïäñ»z¹É?q{ëîÂHÕ?kD…F5à?q{ëîÂHÓ?ïÿír"×>Ûã,ré¸>âÝå)S–>Ûã,rèú'4FGL J1545.8-2336?ځ¹Tòq@8ðgȗÀ:äì-»$.À<a`'÷–¥@"Xײƒö?øpDÖÉ¥Ñ?ў@}·÷?Æþ<"¿j?óYæ/tb@3Z™©‰Ò?Ð0ÿV·È¿í¢FF5nw¿âJßO0j¿¼R—|ˆç›¿×,àÞ§•±¿åï!öÊÍAGNbllNVSS J154546-233929?ïù'6ŽVV?B†]½òô<?I÷%Ʀª2?B†]½òôE?ïýs—˜?U4ë»0«?7g;C=û?U4ë»0¬?ïÓ×£G¿2?wȟ^%?v.\ f?wȟ^%?ïÕ'I`G?e˜ØT`?ul[OÜxî?e˜ØTe4FGL J1546.0+0819¿ÝÇ á/8@FVV>Ðö'À9¸ÀûÞ2PÀ<)µÆ 
b@×-¹÷ˆ?ü¢HåL"?¶íz—JßÍ?ºÀ‹J÷J$@J˜Yþy@…Éy±ì¿äz-ô/¿âDx4Å«¿ÜYˆœò®¿Ð™:¤É¿ã*T'8T¿ÞÊ^=M'AGNbll3FGL J1546.0+0818RX J1546.0+0819?ïõ§‹V'?Se{øö?T°éSÄÝe?Se{øú?ïñd8r¯.?pÖ
R±È?]7¡£þ?pÖ
R±È?ïÍÈáT?}Îfo¥iD?yðùV?}Îfo¥i>?ïBŒìÉ?ƒ³ÚKÍ¿y?ŸNW®bg?ƒ³ÚKÍ¿x4FGL J1546.1-1003?í"Y`p†ä@@Ó£"¯WqÀ:°ÐíÄÀ<1Y²"ý[@ bû0bsh?üqÖ¤?Â&ÂaŽæ7?ÄG0€¦Xš@ú¡ÿ™¨³@\ބ\?ït7àAØ¿Ùñã݊Š2¿ß^¡Ëí)¿Ô¤ô^N¿à½çŒk³­¿ã4…
š¶AGNbllPMN J1546-1003?ïû4°ÄAm?<EKŒ?C-<îúH€?<EKŒ;?ïüÏÛáòN?OŽÕûß?9 ðm‹ª?OŽÕûå?ïÆ
Á!3?~´vøsÝ8?|÷zŸogg?~´vøsÝ3?ï÷··ØwS?<Â\K¸Ú?POZù?<Â\K¸Ùî4FGL J1546.5+1816?Åþ"Ëâ6n@Ho"5ÒIäÀ;¦¸¦¥À<€rmæ@û•b'g@š¸–ž=?ÊçæٓZ?Ä2õö'Â5?ö+—]7@úx3ÃPø?ÂË>Ø,ý¿ÛeEÔö¿ÒZGòÝÙ¿ê\žÊù¿ÖäHŸ+(ù¿ïÿ×ñÃýAGNbll3FGL J1546.6+1812MG1 J154628+1817?ïÆRaßì?€(2\uY?|ÖñO
3?€(2\uY?ïývJÉ`Ž?Iåõô7??4M©´ûŠ§?Iåõô7I?ït-ü$È?ŠSw/{dÍ?'z@|[g?ŠSw/{dÍ?ï¼xõG~r?k
ë
[»¸?€á® c³?k
ë
[»¶4FGL J1547.3-1531?Ã;x-Dw@=¬€ù£wÀ:ÛºÌð;À<kx(/Éò@!&öÝÂhp?ûTÙý6ø?Ô<Iý·{?Áõ:i³Lô?ò'r…X™õ?ù4Í\i¸U?ä¡ìï'{?çJ{NTø¿ßõ¯¯…")¿äÛî=_Üß?ÅGõâ𥚿åTh!§o›AGNbcuNVSS J154725-153236?ïç-µ´5‰?kýwð•K?hÒJKÊy?kýwð•K?ïëôPîV?…sl睰Õ?d¯ùª‹?…sl睰Õ?離•ûT5?ƒøó	¡¸?†Z*ò–?ƒøó	¡²?îù÷!­4?"-¨,? `å,¿q?"-¨, 4FGL J1547.3-2802¿Çôµ8‹0@4‹eˆUÀ:FäH•À<?,˜@ ¬Ùuҕ?ý¡ËFºÏt?½#Ë6I¾? ›_æ?æ̆'ø?øC®®(ÇÊ?îÎQfúàÜ¿Û'\:h‡¿áê9Ÿˆñ׿ÜÛÞaÔ¿ßS…
EŽ¿¿½¿¾œ]nAGNbll3FGL J1547.1-28011RXS J154711.8-280222?ïð©µô{?XÉbÌÔd?^¬"Ý?XÉbÌÔh?ïÀ0QBö?'Tˆ&"ò?¿g×^"Ñ?'Tˆ&"ò?ïÓõ@Ø?zÒ~¥›î?v_üv ?zÒ~¥›î?î-±ˆðÊZ?'ÜÂ;¼G]?­$çpóZT?'ÜÂ;¼G]4FGL J1547.9-6403?í¡³ß'B˜Àþã'áïtÀ:†ƒ<`À;Å%ƺd@ò·É°b´@ßå®E"?Î
èuõ¥‰?Òþ¥¢fqÏ@ˆêb		"@ƒ&uµŽÃ?ï·Do›™N¿ã~Qª¿_¿ì&×¥mã2¿ãlja=1º¿ëcՒn,.¿ïþ|AGNbcuPMN J1548-6401?åÜuIæEÖ?ÊÄá‹Œ?ÔGl3tR?ÊÄá‹Œ?æO}tܶi?ÏæhóÔ%	?ÓaF"-?ÏæhóÔ%?ábá>ï
 ?ºhìe403?Ý:='!ëÀ?ºhìe403?࢓ƒ*)r?µØ*/Y>?ÞºØù«­?µØ*/Y>4FGL J1548.3+6615?ïòä¬ùÜ>@E0å£]gºÀ;—¸`.>À<Çç˜*-Ñ@bÿ"	•*@árƒ«Ë?Ãà|-Q¿·H"ø¦?ñrרÈá†@Kžuvy¯¿½;~0\"¿á³—!U<¿ë»G¿1X¾¿œ
F}Ë¿ïÿ¬ž5¿?ïýÝ`˜ÇAGNbcuNVSS J154831+661632?ïë>á¾øÁ?cîuÙbS?dÁA?]?cîuÙbM?ï•ãؾ.^?¯Ç? ?Š‡	Ðth|?¯Ç?Ÿ?w".ƒ?Š¼1J€?œâô_?Š¼1J"?gø•?z¤OŒž­?€ž;ÁÚ¾s?z¤OŒž«4FGL J1548.3+1456?ëÀ0'Ò:ç@G˜–gµñ¿À8ú‡Š£\'À;É>»ýq°@'gh™ò?þ¼#1]p?¨FΤs?ºäÄæ#Šõ@uâXOL@Ý\ª%?ÞÏh=V!Ë¿»N®ä¯l•¿ÞSa;":¿áDÑöØ9¿ã^[`m~¿åÁ‰¢«'AGNbll3FGL J1548.4+1455NVSS J154824+145702?ïü¬ZäÌ?7ôì,Uû_?:/ÐٚŠ?7ôì,Uû6?ïñ!1‡@?uŁ˜ü­E?]罜ñT?uŁ˜ü­F?ï•~%/Θ?Š‡òûO?Š v´Yî?Š‡òûO
?ïÁÚÎar®?e±»iP?˜ÏF©4?e±»iO4FGL J1548.8-2250¿ä—'v¶@8,Â?«ºÀ9vh<)|À;ÀŒÒá¹Ä@ â×býÑ'?üâh?"z?¬Ï˜ü]* ?£'£Ÿæ?÷«&[´@
6¼ÕˆÞ?ïÿû-2h2¿Ì—Û´q6¿ÑWå.Ãaê¿Ù¥"Ï7á¿Üêö¦""¿Ô΄þ"?AGNbll3FGL J1548.8-2250PMN J1548-2251?ïþÙì»ùO?ªýîk1?"a4@kÆ?ªýîl
?ïû¢.:öþ?Wócã©#?AwG$
l?Wócã©2?ïã4ñO@?s'zžõv?lËæ°À?s'zžõv'?ïÔé£j±?b	oìÔ/*?u‹.Jö§'?b	oìÔ/%4FGL J1549.0+7846?î¦p8]–b@Ahšþ§±À;çÿ:bËÀ=&(
á'@ ®ëA'v?ÿ³ø`îW?у¤D˜`_?"†`ƃ u?¼|`"Õm@¨ÊÈ»›!?ì¼]\Òi¿å­½Þ€i¿×¾¤kÚ¿Û逢&Ûâ¿ã;ýÂ8T¿Ø;Ä~AGNbcuNVSS J154837+784526?ïþ•¨.w=?$õºA§xL?&¥}Œ/X?$õºA§xÕ?ïþç¹2£­?:В.g|Ë?!"lÕÅ(.?:В.g|è?ïò@›äÃ?q¿\†%C?[~È6y¨?q¿\†%A?ïúgQMº{?4ŒI­.å??FbºÉ×?4ŒI­.ås4FGL J1549.3+6310¿ìZ"e4@Eô<³åuÀ;NÊW§†ÂÀ<f<Àz®ó@Àe©}y@>Ü´¡]?»^ò>Kj7¿Â¦jŽ.@ô<¥¢¼X@¯:¥ÃH•¿ÖúüDÿìaðµà!=¿æô'¢TS>¿Ñ£ÌB¹8¿å€|ý ¿Ý¸ƒÕ6oAGNbll3FGL J1549.0+6309WN B1549+6319?ïý8Kd?7¹Ìï¬?7×æ=¤Õ€?7¹Ìï«Å?ïùÅ:G]ˆ?fafXâ?Hëâ‰à?fafXâ?ïž]>ì+h?‡Òï@?ˆh°Dõ%æ?‡Òï@?ïé<È%Úý?`.Y²ðB7?fÃ7Ú%v?`.Y²ðB74FGL J1549.3+4234?ÞAôu³+ª@IsŸ©~+À;Z|Tå5À<ì¿\¢˜@awcä«ç?ÿÛãõhÍ?ɘÂçÇ?¿^Ðߚɉ?öH8c܊@\­+qÈÅ¿ï§î'‡Ù?ïýk›Y:¿â™ÝW‰¿ål妸f
¿Ë.×XìÖ-¿ì¨Ä¯ÇÙAGNbcuSDSS J154918.64+423500.6?ïígïPà\?aÿjȏ$Ê?b˜¯¤R?aÿjȏ$Ê?ïúº=xå?_¶™Œ?EÞmÁ?_¶™Œ€?ï§a¸ó|?'œÍç ép?†;ç'Ã!b?'œÍç ép?ï½2¡ÒÁ?p¾ãÁá?€¾3W‹P?p¾ãÁä4FGL J1549.4+7409¿àâð7,'@BÜÿ—$tTÀ:¾‹ƒVa6À<±òeÊ@ Œ7Ü:S@EÖٖë?ºw¼úò¥¿®sìôQ?òæY¶T»C?ûn3´ãL¿Ù¢¥œ\AŸ¿åü†™Õ ¿êŠwB+ɇ¿ÒײÄbðæ¿ééâ‡I4ý¿ïþS!æÕAGNbcu3FGL J1550.3+7409WB J1549+7409?ï³èõ2œ?ÿ*Ƶ\?ƒ³X܎?ÿ*Ƶ\?ïkÿ€U!Ì?¡ç&up?'€õ[ƪ?¡ç&up?ïe.°<$^?MO·Nk?"Z)ø{t?MO·Nn?îy;¡•0?—G¯$Ù¯'?¨n,Eæ­?—G¯$Ù¯'4FGL J1549.5+0236¿ÃèõЂ@DqÔbÃC·À9%[ÚjÀ;ümd‡i@ôÊöˆÞ@òÁmóùb?«ÂÑBÊ¢H?®Ú€Mœ@háa«@¯CWË[¿Õê0_ï(í¿å@ß=è˜Û¿ä¢i÷ë_¿äȖ<"¿ë´	tC¿ïúÓÍ$áAGNfsrq3FGL J1549.4+0237PKS 1546+027?ïúÙ|{?@ƒ,‰Úrc?D›Îø`?@ƒ,‰Úr]?ïü}ïI¥Ê?R±J^è?<…²Ñ²G?R±J^è,?ï°2¡®ž?"zΦú?ƒóW"X{Þ?"zΦõ?ïýzðÃÅú?'>´ äm?4(yáÐ1V?'>´ älÕ4FGL J1549.6+1710¿êxšJÔ@Gä\ÈWóÀ;%–'~À<"íٌÏ@½³Wô†@'T·?ÁlIªC
¿¤ú [Ùß?åQ‡F°¾y@— t>Á1¿¶|n¨°¿èÀ*'_–>¿ãÐÂOpV¿å2Át‰À¿ÝËŸŠtc¿¯Öa"iAGNbll3FGL J1549.5+1709MG1 J154930+1708?ïþMþBãT?"S¼Æ=Ô?+ Ñʯ_?"S¼Æ=Ô?ïýßëÛ?L»•¶'‡?3y£%ž?L»•¶'x?ïö²Ö¸¼?bðœì1?S̚RŽ…¤?bðœì1
?ïû썼?1¥@ª»)¹?@O‡•É@?1¥@ª»)·4FGL J1549.8-3044¿ïâ"Ú4†@2' d#–À:§$WÎ/À<h;¤ñ¼p@!"ƒZ=
?ûñLÞÕãÍ?Å/âç¸?¾l͞-ýê?ûŽÍ=5µ@f?˜ò)Ô¿¨è7Œ^H?ï³!ž¶9¿â[ˆAWŽ1¿Ò‰ÞÛÃ	Õ¿ÕJҌ)nŽ¿å-4±B-AGNbcu3FGL J1549.9-3044NVSS J154946-304501?ïêlqçÌ?d<Ãb\Jï?eᓎ5?d<Ãb\Jò?ïëîàʬ"?€(La‡±?d5SÝ£?€(La‡²?ïق¡ˆÝ­?ròÿÈÛa?s>¯;')é?ròÿÈÛU?ïáÜÑs‡?‰r±l…z…?ãÄeя<?‰r±l…z…4FGL J1549.8-0659?ÕÌVþ	Œ@A}j@ºˆÀ9=+úYÍÒÀ;ç<³åu:@ÄO(1L~?þ­ÛÛ]‰H?®ªq>lÞa?':Ǭ?ðÄ öð@¦®<éÀN?ï] Å¿Úó)âÙ¿âŸÒ}浬¿ÝT]¥L«)¿ÛÒ_qÕÛ¿Ú@ŽERš'AGNbll3FGL J1549.7-0658NVSS J154952-065907?ïú°/L5?A@–ÑBé7?E?BÎ)ƒ?A@–ÑBé=?ïûízɇ?T€×Ö«?@JÙ㧲?T€×Ö«?ïîAmá+[?lyJ^uÛ?a¾'Ô¤?lyJ^uË?ï®Rö¥Ìc?oo'yqÌ?"kBVŒç_?oo'yqÇ4FGL J1550.7+7006¿á6ãÝêR@DjËGÀ;@öý»'À<º7ŽÆÞ@<Ÿg™?ò9ìxkL?ÛtiÉÈ5Ž?ïþMþ"7@O×^ FÇ@úL+&Ê?î¶Q•ôÉk¿Ýä©ÍÄC'¿âèj{€)¿ïg/ò?M¿ïŠÿ…†½¿à(6îÎAGNbcu4C +70.18?ïËDífRa?Š´Ö‰w?%?z]‰LÖÏ?Š´Ö‰w?'?îÑ(WÃÁ÷?½µ¦|㪝?¢ízƒÃà®?½µ¦|㪝?êçÈïG?ª5äõ?Äc ÜCšç?ª5äõ?í1…¨?¯ªíŒóÉ?·ÎwóÒ½?¯ªíŒóÉ4FGL J1550.7+0528¿Á~»:Ϲ@EˆÁÛCÀ9œÊ
Õ«™À;ç þ}I@—÷û#Í:@,џšd›?´VÏÅzž?Ç÷Øi8'å@þ‹;26@
èØqÊ?ð¿ß'ü—?Í¿äD£""dS¿ãä'Ë÷º·¿íju>ÆdS¿í4€Û\²ˆAGNfsrq3FGL J1550.5+05264C +05.64?욺®ÿÍ¥?¸IŽò:;?»**ˆ'Ó?¸IŽò:;?îº36Ö0±?¶ëÐòšF?¤\̒œôø?¶ëÐòšF?äÐw¤_)º?µ1#èÝT?Ö_·A¬Œ?µ1#èÝT?éþËjÁÓ-?¥~;ÜD?ÈÒTø³K?¥~;ÜB4FGL J1550.8-0822?ïzã ~@@ól½˜|cÀ:ÏR]šæÀ<i‡¿}@!I³	,N"?û¬Ÿ¶Lä?ÒûOyx?¾G¼,@¥¸?ñaI["¤@/—b1ÎY¿ïh4œ¿¾Ç?ã#Mâáâ¿àYÕÿ{u¿â˜TTëꟿÂð@uœå¿áÍâ½ÐAGNbllNVSS J155053-082247?ïÿ 5ì?/%¡Šþ¶1?íùBnNK?/%¡Šþµš?ïý¹ô´4U?R؛°®áà?20Z^]`¢?R؛°®áå?ïâ0²dÚC?sÔÒ`QS?mÏM›%¼Q?sÔÒ`QS?ïð[mZ?R¼—"dm?_I%Kîçf?R¼—"de4FGL J1550.8-1750?ïìp<W/@;oyB=À:f<OšÀ<#PÐÒëË@üZ.Ì@¹cc}?Áꀘ@Ô?ˆ³xy¶
?Æúw•bÓ4@Šá^<K?ïÿ|ý¬"œ¿æ/N6ĸ+¿åÊWÂ^´Á¿äBÞ6œM¿ïlbäѦ?ã£æ#µèAGNbcuTXS 1548-177?ïñÜ;·?^Õ eé¡Î?\Gˆü'Ø—?^Õ eé¡Õ?ïûŽ‹M?]!¸9?AÅÓæËÓê?]!¸9?«ÚT?">ÇŒMæ?‡Y•	jþ¹?">ÇŒMâ?ïß@–¡?aÐ
åÁf?p_ú4¯vŸ?aÐ
åÁi4FGL J1552.0+0850?ítJ®QŽŽ@EӜZzÀ:E`Kš2FÀ<b«esø@Æ;óS?ÿƒ>Éijþ?À6+ágC?¿9òj@ƒaŽQ@	ZP1›®r¿êÒ×¾Bph?ïå
`¬B¿Ý™–ÿáL6¿à6çó™À0¿ãš¯ú./¿ê71Åté·AGNbll3FGL J1552.1+0852TXS 1549+089?ïü™N ?;<qû¥e?;5ÆÿG?;<qû¥¡?ïú3q¢I?\zag	?G28õvÙ ?\zafû?ïá¿éÕ·D?qŸt ?õ?n@*Hº¥?qŸt ?õ?ï¯f‹îx?r³ÞQü¼‹?";æ]aæ?r³ÞQü¼Ž4FGL J1553.3+0600¿íصc`g@Dù‰7KƨÀ;6Yì yÀ<"¬X¸þº@®qÔX²I?ý7÷¾?ÚWÌOðÙ?êPåË¡T@¹àF&Tþ@ËBhÛ5Æ?ÕÔ:ªJí?ï•÷¹	¡i?â+@š$¿ç²_ä@¿èÒGàê;¿ïú~¯"®AGNbllNVSS J155331+060143?îìCt>×?¡;ìµcƒD?¡>ȼŒ?¡;ìµcƒD?ï{yìw?ªjõg+ˆ?ŸÐÂq?ªjõg+‡?íCÃ>¥<ù? "O3˜%?µáæ
ÖE? "O3˜$?çím·?}?¶

L¨T/?ÑÖ%$'?¶

L¨T/4FGL J1553.5-3118¿ï—Îåè¬ù@12—9m	À9Z—ü
¨À;ÃxØXò
@aÖ©?ý'RÛo&ÿ?«M—@+œÄ?µxs'-Â@
žÏc€@S¾	e"i?ïõäRûO—¿Àßȧú"¿ÞÚ/H¥5¿Û˜™ÿÅój¿àÑâœ'¿á`‰ƒœAGNbll3FGL J1553.5-31181RXS J155333.4-311841?ïýŠÞbç?+Ý=⹟U?3©èÇËÂ?+Ý=⹟g?ïò냭£Ï?m<–,ëô?Z(ø¤¸aÁ?m<–,ëô?ïājôS?TÛ«& n?}ž¿J…Ö`?TÛ«& l?ïԂCrW\?_«a¼Ÿv?u¾ÞFÔQk?_«a¼Ÿu4FGL J1553.6+1257?ÎÇûM…@Fš½çXÀ8àPšLGÀ;ÎtqÁä;@ïSpÁ@_æ\ÀË7?¨¿!œž6?¹ÏòF.®@
'âûã:Í@÷['¢Ú`¿Ú"
P»Ú6¿ãÖGj!ÜÊ¿â÷škP°ò¿çèŠÞ?æË¿êOP ,¿ïê=@RUAGNfsrq3FGL J1553.5+1256PKS 1551+130?ïùQ²e*Ã?Dën
|í?J¹6kTó¶?Dën
|Û?ïú˜$©¥…?iwSSl¤?EŸmYië,?iwSSl§?ïD]ìøk©?ïkÙ¬¤ñ?—tB`òŠÖ?ïkÙ¬¤î?ïÿ§Òä|
>ú¯øMæŽ?Fàüª³>ú¯øMâ4FGL J1553.6-2422¿Û+
\ºÆ@6OÙÛ©¢À8²
RÎÙíÀ;Ëãktà @\ê«Úä¾@sÄóºw?§MìGŠ½?¯)PÂvm×@iÝcóÅ_@}ø¸¸îŸ¿»aX"Ì¿àڏbÞòi¿åL'jP¿ãGÉÃ-Ú¿è{ß@í±¿ä@Ï_~AGNfsrq3FGL J1553.3-2421PKS 1550-242?ïóG'՗?T´Y«[=Q?YpûÒTÐÏ?T´Y«[=R?ïúîyZ"?g¦Êº/(?G°F•ì×?g¦Êº//?ï½g'jœ?|;K-×?€¦y¥Y2?|;K-Ù?ïýÞõpι?#šýÆl?1TyŠ,w?#šýÆ4FGL J1554.4-1215?çÀ'V5>@>¨îÙ8À:­ÓÿÆõÀ<S'üžK°@!!šû™hò?ùÑ÷®ø¦?Ñ"ð½m?ۅlÜ!S@pŸ±@NoMjÁë¿ä3ÍêÙþ¿ï®3ïñ•?íé°"G'²¿±ìµàÍ	Þ¿âҊ¡"³¿åv_¢ýÆjAGNbcuGALEXASC J155432.61-121325.7?ï²J©"ÌÔ?}%NÙ	
?ƒmUžÌË|?}%NÙ	?ïêÕá*¨?z¶¶ 9½/?eä*ÕX&?z¶¶ 9½-?î?Î<»UM?¡gûÌ)½?¬4J«:?¡gûÌ)½?î1eÀ‡?rƒÙ²œ?®þé£÷ƒ?rƒÙ²œ4FGL J1554.9+2143¿Ë²Ý{yÒÇ@H
uÍ·À:ºà¨KäÀ<'sϵq@ënºGäñ@Ât֐›?Ê<Kö"±†?ÑqP¥4@‡Š£\û@ó…mèÎ¿éòUóQ›Ô¿Þ¯ë¶pj¿Üž'¨'Y¿å×ï_ô²D¿æITrHù¿ïåXÿöoÞAGNbllTXS 1552+218?ï¡nE¢³r?ˆkn_":û?‡¤n—S$?ˆkn_":û?ïøg­»šJ?cŽšùκu?NaI–Ô"?cŽšùκs?í'ÆÌc\µ?¡dÿZY±S?³qɜåS?¡dÿZY±S?ï#g'IS.?'Ã)\ëµ?›"՚2?'Ã)\ë¶4FGL J1555.2-4149¿íÔfïç$@"
?·¥ôÀ9eR1%;úÀ;rƒ]œ"@š–pÅ:@eÐÄ©Ý?ºB÷ ˆ`·?ÈÏÒ»¤0v@üÿý@öQ'S?ïß¹£ûk¿ãâÑñÏ»•¿ç†‹À)M¿ç|ŸÃF1¿ç:hŠ'¿¿ïüÇ0«™vAGNbcuPMN J1555-4150?ï˗ÙÐ'?K©ŠÂ?z4uìò?K©ŠÂ?ïæÇ\¿—v?ƒÞ;ürÕ²?i8£@h‰D?ƒÞ;ürÕ²?ìåüUª²?¤f£H9n?¸ÐRªp?¤f£H9m?ïyÂÈså?{°æW9ÆÝ?Ç¦ñ#c?{°æW9ÆÞ4FGL J1555.7+1111¿ïã¶"Ul#@Eû~|âÀ6{Ãiv¼À:xßN¯|@üØ®,x¯?ø¨–<"?Ž¡öVÖGí?±cXÊÇd@¯b_p¨à@²‡ªƒÌ©?Ù͵à¢Á¿Íù2±-4¿Ö3=ú·k½¿ÐHÏÃL¿ÙQºÀ/Û¿Ù.šG>'óAGNBLL3FGL J1555.7+1111PG 1553+113?ïn'W'š?­uj˜Nƒ?'-ÕÍ?­uj˜Nƒ?îóÆÆoä?·Ö+Vh? Ã"ž¹¹?·Ö+Vh?íËÄü£)?¥w®'Á?±¡Øçî¹?¥w®'Á?éþu&#ë?²›ÐRC ?ÈÂ+gpR?²›ÐRC 4FGL J1557.5-7040¿ïáÈE¬i§À*Odñ`¯À9¤Ãð…8ºÀ</)¹6íÓ@ąrp4ñ@ƪ#T˜ß?³îÅ`ß$?±7Ä<…lf?ýQ‰)ßÍ[@Ž88€¥?ïëÿ,›i}?Öwz?·%¿äV4ŸÄÖß¿Þ»#­Y¿ä5YžVí£¿ænC?ñCAGNbll3FGL J1557.4-7040PKS 1552-705?﷝+{?€Edó@¶?'?µ?¡K?€Edó@·?퓩Œ¹b]?À‰õ_R?³b³š4í?À‰õ_R?ïtI~ ?Š?ïÚ
Œ,?'|]vÐ;ò?Š?ïÚ
Œ+?ê¿Y‹\—?¬K<^gúE?Çřҍ£?¬K<^gúE4FGL J1557.9-0001¿ïƒ2–Ðþ/@BÔÝÖàLÀ:®]Ywj›À<3nUH0ñ@¾x,a‡Ú@ŽÉ¹òÕu?ÑÆláTÄ(?Ê5öHÇ?õ.éÝ~˸@hØë>'¿äùn‡P¿äÏ© ø³…¿áNƒ†1ÝÉ¿ä­¡ŽZ¡6¿î´²ú"¯¿ðAGNfsrqPKS 1555+001?ïí'ØüÒJ?d¦uc—ØU?bØ'-¶?d¦uc—ØV?ïøØè3à(?t&M
™'è?Lœ_0^³?t&M
™'å?îàƞ?›ÜPŽj"?®.qÿC–#?›ÜPŽj"?ïÍQRx#?f‰9BÐÅ5?y|WVÃî	?f‰9BÐÅ14FGL J1557.9-1404¿ª"p³@<Îü›ÇqCÀ;ä܎
ðÀ<¥³7ÐPæ@ë%ŠÔù@U—Ià?Ò)õ1oä"?èQ¤7'M@›ß°Õ @¥õ¢"?ïèçë6D`¿Ï¨ýz>µr¿ÆQˆöÄm¿éprž®"¿íTÝ!®¦q¿ïþÛrýœAGNfsrqPKS 1555-140?å=RØ"Ð?Èï%H'k??Õÿ…ZOº^?Èï%H'k??à¿ÀØîM?ÔÊʧ«^¥?ހüN#h?ÔÊʧ«^¥?ã¹Ât£á:?º¹íën0)?،{¸=‰?º¹íën0)?Ò-ÃY¬?®i"è{ ?æéS)ü¸?®i"è{ 4FGL J1558.8+5625?íÓ YJ
r@Fá«\9¼ºÀ99¿×hÀ<J໗@Ÿy•în@iåŸ+©Ò?¬þ¿õ40?­$g_×ùH?ýFÈ •¡½@Úœ&g?ïÌÔÉ'¿äÒ`v¸C¿áÃq~óP¿Ý$O\^¦¿ãwomv% ¿ïÿòß0&¹AGNbll3FGL J1558.9+5625TXS 1557+565?ïþël0r?}2Ó¹?!I>ÜøÄã?}2Ó¸Ç?ïûRñxt?V¦Œ"#6?B·Ü:-æ?V¦Œ"#:?ïâ‹ï³P?v¸SÚ¥?mtæL¯·?v¸SÚ¥?ïê&OK&´?TôfâËi†?eÙ°´ÙK¦?TôfâËiƒ4FGL J1558.9-6432?áykÆô·À!F‹;26À8©1½nÀ;ÒêVJp@²X>…vÍ?ÿA9k[˜­?¤âb¶-¤?—Wºã&'?ñ²žÓ•=ê@פ"G ?ïíH"-§X¿Ù	ÿ}y'‰¿àS™Û¿ÞSCο஗WŸú¿×uq{î8AGNbll3FGL J1558.9-6432PMN J1558-6432?ï÷=q9ó?N˜lêI?Q…ŒÞL?N˜lêHæ?ïèŽTø?ðã‡öZï?gäqü«'?ðã‡öZð?ﺠUbæ$?‡8'ßâ^#?Wê§Fvõ?‡8'ßâ^#?ïBŽ¼™"?…m/àÿóy?—®(LÍ´?…m/àÿóy4FGL J1559.1+6736?å""è"­r@DcEŒÒ
úÀ:ö*rDÀ<á‰$@›½Ñb^?ý…‹ûKeY?ŝ^J82v?Â3Eèª;?ú®ç¸5f@M¥ÿX¿Ú(ç	D¿ê¡uÁ"I¬¿ÂA…±ZV¿ä mòKâ¿ÖV>{ë°¿âž8ÀúõAGNbcuNVSS J155856+673646?ïø ÛÛ Ò?Nñ˜Uـ?O|"|¼Ë?Nñ˜Uـ?ïý´ËL}?IùÁ#uýý?2Y¥œÿ?IùÁ#uýþ?ïÚcRÖîQ?w'ð×!?rÎV"ˆ×Ò?w'ð×!?ïêÂMpkœ?R*û†îÅ?e=²"aó?R*û†î·4FGL J1559.8-2525¿åô(t¾@4'"àÞÓÀ:^ם
gbÀ<#¤¦©M@éш'›@r=Ÿ¿™?¾húÀP¿ˆ(ÎÓO?ÉÏa<0@|ža)'¿ã_¿"å­¿Åÿ{&<¿çL_ß¹Ž'¿æü¿ÔKK'àD¤¿ìSŸÍ:[AGNbcu3FGL J1559.8-2525NVSS J160005-252439?ïÄÊëR?†?±óÃ?}šŠVôö?†?±óÂ?ïý™GÿG¦?P"œ(¿f?35ÀÂÏ?P"œ(¿]?ï£×ÆÙ$?"©%Aºi¿?‡
I¿÷b?"©%Aºi¾?ïô½ðVû_?H…né
È?V"R	C"?H…né
º4FGL J1559.9+2319?âžPÇÍÿ@G¹I¾ó(À9ßÛz¹×À<<¤:Œ@7'&«;@^ÁVw?³dŠn-…?q½
«Óò ?¾
~BÑ
õ@
æéI?ê§Tm@?Ý¥h"αS¿åŸÁ}ä1¿ä3aÁ»÷'¿×áËÌòŒz¿íÙ®'O"}AGNbll3FGL J1559.9+231987GB 155744.0+232525?ïç@]eÓ?a›Q°DMX?h¿¢š,é[?a›Q°DMX?ïü"<þgW?Tiÿ*!©Æ?;fÅPÁ?Tiÿ*!©Ì?ïµ{ߺcØ?Pe©OÆ?'¡g	þ?Pe©OÄ?ïñy1L³?NÈý˜Ò˜v?]
f™òÎ?NÈý˜Ò˜ˆ4FGL J1600.0+8510?ëD7Ò
Äd@>Z_¦XĽÀ:š""œÛÀ<Š4 ˜ü¼@tÊUú˜@bÑ6¿?µÞj(ÿS?¢¤Á¦?ë•ÏªÍž"@9"í];¿ÚÜÒČ¿ãÓșae¿áÚ¢þ)q¿ÞacÝu¿áŸÑâ5iÄ¿ìÔUøZQAGNbcu3FGL J1559.7+8512WN B1609.6+8517?ïò8LVþ?U€ÛKÞ9^?[gRæ9?U€ÛKÞ9^?ïü­ˆÉò)?SԜ$Ûâ?:"¹°n®,?SԜ$Ûå?ïÜñA1¿?x¿}Âτ?q‡_gx ¾?x¿}ÂÏ?ïǨCï©?h'>À›£?|+ÿÞ+N?h'>À›£4FGL J1600.3-5811?â:¤"|/=Àœ¾|§ñKÀ9²~'ÖV¹À;³lsÆ¡:@$-"$@©öùÇÛ?¹H'OÐø«?Åz‹vì›@
IˆÅ5ÿ–?ñ˿ɯ?ïýqz–Ÿ?á`·Ð¼E–¿är4ÐÂ$Ó¿á™«ßí;¿çO ~ûˆ¢¿é(ž[ÙAGNbll3FGL J1600.3-5810MRC 1556-580?åëÙ?æ~Ã?Êêib\%?Ô(M€3z?Êêib\$?ДpVpE¥?Ñ=0uâ?çµÇÔÇÝ.?Ñ=0uâ?æ‹ÛŽâ8?µ®ušjܟ?ÒèHâ;Á?µ®ušjܞ?ªYêîR•o?"3´ÕÀp?îZaQÖª?"3´ÕÀp4FGL J1602.0-0641¿è𘉽Ã@@lÚãæÄÆÀ:ÃÌ­ÃJÀ<J¶¶^Ì@\ÕOÓ'@p̆Uï÷?Ïz4y"P\?Ò_Û\Ý{œ@×z€ÎÇ?ñ"icñÁú?ê¬aBD?íAd®L¯¿á-¹v®³¿âñ.«äö¿é–}_Ò"¢¿ïþ¢NZAGNbcuNVSS J160146-064256?ê"îÏ3‹?Ä';Î2È?ůìDÃ1Ö?Ä';Î2È?â@@Ë"º?Õ-;ªEa'?ÛÈiº‹?Õ-;ªEa'?êÒ´_:H\?ª…Uêñ¢(?ĵ.ƒޑ?ª…Uêñ¢(?Çý;)xlf?®™Ç7¼Í?ê±5¡äæ?®™Ç7¼Í4FGL J1602.1+3324¿îÌþL#–@HZõÊÀ:ŽFipÜâÀ<¨´ú¬@×	µ5l@k¤"ÈŸA?Á8ø²<(?¾â_&ù?û‹­b¤:@~ôþð
•?ï¥^^Z(k¿¢ÃÂbÀ¿å¯Ö(ôì¿ábòsO'õ¿çÌÀ7"D¿ïõµ>:Î2AGNbcuOS 300?ïWÝT?•fâCñsx?ª>HºêÚ?•fâCñsw?ïæg)£›ª?~|ê5C)¥?i˜Ö\dTf?~|ê5C)£?ïhµdj–?ÒÀmêC?'þ)Sr­0?ÒÀmê??î'Î<0?"VïUH?®
ƒ<÷ç?"VïUI4FGL J1602.2+3051?í?^ÓY¥@H5Þ½çÀ;¹†žëÀ<¼}ÄY@×kÖïí@mç˜ã?ÄÅd"¿H¿¢ã	'¾>r?ý/|&ìþÆ?ïîýy=¿æÊ?d‡¿á5tV2¿ã0‰4LJé¿ÔZe]Që¿ðAGNbllRGB J1602+308?ïõú¸ît†?QUôë†	*?T
Ž#óU?QUôë†	%?ïùMvS?e<µQ[âÅ?JÊ'¶³¿2?e<µQ[âÍ?ïÑÅœ?z°¾Ó¤º°?~7}2e?z°¾Ó¤º¶?ïÀ8Žü¿x?l'‹*p‹?㸁 C°?l'‹*pˆ4FGL J1602.9-1928?ÙújވRn@8C(ÃnÀ:5s"u"*À<([{PÙ6@<MŠ!…@\ޅ[ôó?Òõ»ƒyG?µp$À©¨Û?ò¢êÊ
Ö@ŒrêƒA¿²#½tj5(¿ã6 M}aU¿á4DZ°è¿Ú"UÅYeø¿æTÞÿQš¿éUõÀa¦AGNbcu3FGL J1602.8-1924PMN J1602-1929?ïü¨³CÏ?3eǖ|M?:ºg…á~g?3eǖ|Mb?ïýÀ5ÿÏ?IM ׯS?1ÿÖPˆÃ?IM ׯI?ïõû¿g·?cÙXwvý˜?Tï0""?cÙXwvý?ïâN2é1?S³È&ÞÁ–?m±ÍoÍÜ?S³È&ÞÁ™4FGL J1603.5-7112¿ïßåä ÀÀ+đ)ˆ†À:¼ÿc"HÀ<3`:Ó:¥@*Ÿ"ƒªð@û¯S?B5?ËÉB	9å?¹¾'ø?Â8?ñkŠ'•™Z@¯ËE¥Q?ïü	 ?
¿èâÒþ?5 ¿çE^í{Ä¿à–±RF¿êtjÀ¾ ¸¿ïþ°à<4AGNbcuPMN J1605-7112?ï󓭅šÐ?[3˜"3?XؤôÊa\?[3˜"@?ïÃ
&¨Äø?'RˆEV4›?~z쫝ƒÐ?'RˆEV4›?ïgMçN—Ã?ŠtÓÕª¹?"C-²?ŠtÓÕª¹?îâjÖöª?‡ä1¡7E8?¡ßéR•\?‡ä1¡7E:4FGL J1603.8+1104¿á+t‹(YÞ@Eü'œýÒÀ:¤Z7ƒúÌÀ<Kü²m¥ö@ñ< e'@ð?)á{?Áà;êf政U³·µµðB?™¥Zˆ.@‡hÆ=­¿ïž5_³Cå?ï´øÐ`ֿ暉ÿÖ%¿á%ÀN9H÷¿Ù°L£òý¿èò5ÂY¬DAGNbll3FGL J1603.7+1106MG1 J160340+1106?ïæZœ=?huKƒŠQÿ?iì¥úcÁê?huKƒŠQü?ïýù?G`'…®k?07÷O¡p?G`'…®c?ïӔ1TÞ§?y'mà^Ë?v5çU¬'?y'mà^Â?ïéBq11q?X*fz{ž?f½ŽÎΐ·?X*fz{›4FGL J1603.8+5009¿ïî0wÂÙ®@Gz·ÃPLIÀ: ÌìÀ<§P;¶N@ ,¸¢v³?ûØ	@ñaØ?Âø'6H¼\?Æ1‰Û@ƒÛÂ3?üúWŒ®ÏŒ?鸊à刺Ð8Éà‰B4¿ÅPäÉî¡¿Ûü'œýÒ(¿âK"é\P¿à¿p\‰nAGNbllSDSS J160339.49+500955.5?ï–òY"ã?…á€êïŒ?ŠCižÛÇ<?…á€êïŒ?︺ϕŒ?"þLjî?ÑOœ²?"þLjí?ïužƒÏ?%`¼|?']ì=o†?%`¼{?ëL±™é¼"?¢>	™òR?ÂÍ9˜Yy?¢>	™òT4FGL J1603.8-4903?åK,ÔÀ@›†»ÒªÀ7¶Í׎ǮÀ:¹oó­â&@ 4ÞÁÁÖÐ?þ'ü\'?£Ê`0žj?¯Ab\&ؘ@ŸÆ¤"Ÿ_@ô<ö*"(?ï±ÃŸ|Ý¿ãC´VÝ\¿áŸÆ¿l'ú¿ÚÜéåâGˆ¿à…_L–²¿ßt¤9/ÌAGNbll3FGL J1603.9-4903PMN J1603-4904?ïóB£D²?cåoKÓø?Y{â¹všú?cåoKÓø?ïïŽëì®(?xÖqC÷Å·?`qQØ)?xÖqC÷Å´?î>.‡3Ýè?¢žSëg‡N?¬ŒÂ!~?¢žSëg‡M?ïþa)èa¤? š]l¬?)íayåÓ1? š]lÅ4FGL J1604.5-4441¿árәN¦@­§m˜À8ŸïŽ˜´—À;Žh
/"@_«Jqg@Ez]"?­NÀàãã?µÔšaÂÛ@©ŸâÚU@ÿ]®1S?ïéÌ¢Zˆb¿Ûf&ºÿÅÈ¿æ'f pbê¿âééþ‹á ¿ì,Þ_Ç;¿Ó5nA&:ýAGNbll3FGL J1604.4-4442PMN J1604-4441?ï­Þ?9j‡?‡cD6q?"ˆp1¥^;?‡cD6q?ïõGÃà¡D?p^síù?Upx>½v‡?p^síö?ìÞê£õ'0?¦˜2I2ƒi?¹ªàVƂ?¦˜2I2ƒh?ïùˆ|—p?=›Ë¤U{!?IÞ
¡Â;À?=›Ë¤U{4FGL J1604.6+5714?îŒÁøì‰
@F^4\þޘÀ8¤§.­'uÀ<Õº²@±ÔÎÎÛ@ɐ¢zì? u ŠÜ_?³……žÙt@²¯CO
)@7cI¿×Qaz>¿á¤€-ŒÖ¿æ|fîK¢–¿ä/¥²óˆ¿í•ao0º¿ïÿ "_õAGNfsrq3FGL J1604.6+5714GB6 J1604+5714?ïü½JÒ#?3ó㗗zÊ?:¯‰ní‰?3ó㗗zË?ïçÇ"¿?||'Ã:[ð?h8þ{á@½?||'Ã:[ñ?ï•ÙVA›G?Š°ÂðUßW?Š‰ªo™.?Š°ÂðUßV?ï›îêni:?w9­áø,·?‰Ede±*?w9­áø,·4FGL J1604.7+1734?ïĀü¿½o@FICä/À;(2Æü©3À<£Ø涂Þ@h˜ð§H?ý¨PKqîZ?ÖxŽ·«?ÓÈxª5É@ÖV%¦'¶@üçõG?Z¿ïþ²Þ=°?ïÿ
×ÊVÑ¿Ú%¬!†x¿Ö<« —¿ì¦>Ê.¿ï÷Ÿ¾÷¢AGNbllNVSS J160436+173324?ïìC¶Ïku?jik­\èk?c¼I0"‹C?jik­\èn?ï¢
¦‰´Ø?¡
û7>¥{?‡}V]'Ê?¡
û7>¥{?î;ü5¢6?›¿"!)]?¬@<®eܦ?›¿"!)Z?ìwãë~€?¦Ûìž]Ӌ?¼@à¤ÿƒ?¦Ûìž]Ӌ4FGL J1604.9-3414¿ïðÙBFB¸@*Û=ŽcÀ;D@\çbÀ<}Rkî@!…çïf?ü-Yvɋ?ØÔ Ö¤¼ã?¼'	AóŠ?ì"D¶v$@½_&V+?ÁóAÁ‰?ïÿ§¬_o¿Þ'{%ì¿Ø~¢u¿Ó$¹½üOq¿æ?,î‡ÞAGNbcu1RXS J160452.5-341407?ïÿ43'7?égsˆ/½?yy¹P¹?égsˆ1 ?ïúގï¨a?c'#/(Ý}?D…ÄA^y‰?c'#/(݃?ïçßURmx?q‡D*Ï?h ª­'‰0?q‡D*Î?ïåÎ;Hø?[¢.]?j1ëÄ·¿?[¢.]•4FGL J1605.1-1140¿ÇûùÝØj@=½ƒƒ­ŸÀ:U%t9ŽÀ<,=CWm¥@ 
ä‡(¨Á?þ'Ï…ä°ï?Ç7y©d<ë?È£}É@-gAW¹$?ýîGSP´ù¿ì!"Þ™¨Þ¿¤öw@(d"¿ÏDYKK¿â:¹ÚÁ6¿ÞCùÿàË\¿ïÿy\ã/æAGNbcuTXS 1602-115?ï ±€Ô–B?žJùwªÅ6?›éÏåm7Ü?žJùwªÅ6?ïÑl֟Œ?Št¦ž˜‡a?wI"°rº?Št¦ž˜‡a?íÈ(Ÿ©?¤íoѾy?±¿f»â¼?¤íoѾy?ì¸]ɳ-¢?žïâmJƒ–?º=²f'ô?žïâmJƒ–4FGL J1605.5+5423¿í@¨¬'6^@FƬ![š[À;;¡…÷%À<ém ‹]@ ˆ"Té'T?ú²ÜÌQ$?ËÛTyÿËR?ÇڇËeï?ýšR[íf @ò<˜Œ©F¿ïÿž`¨·D?ïß½4©Tø¿Á0Q"Ñ¿Ó^¢!Ód¿Ý.¿»Â8t¿éÃf½Ë¨AGNbllRBS 1555?ï÷.ãcy;?J¥Àï5ºz?Q¢99
ˆÛ?J¥Àï5ºV?ïúHØe?` .»ñ¸?FÝûОk	?` .»ñµ?ï¿*Vf½0?z±}ݜ‰ö?€5jfP´+?z±}ݜ‰ÿ?rý±Ä?v²½Dë@R?c@"Žö?v²½Dë@R4FGL J1605.8+7208?ånooÎê@Bõ¢ß"xîÀ;â©,´"ñÀ=2OŠÎ¢@!LçÂFŒ?öX¡fítã?×
£|ÇPâ?ÕÁ—Å.ô?ö
e´¿@_°
tM/?ïü¬ž"¿Ñì"xK¿î"'r4Ñ?ä𒤲ÒP¿åÖ<b0÷š¿ÁÕ;ƪžÐAGNbcuRX J1605.4+7208?ïé4¯È¸û?qìÄVÁu?fËP7G•?qìÄVÁv?ïú‰˜—/?fϚx<€?Eٝ£Aú»?fϚx<€?ï~}pì·?‰Û•MÜø?0QâiW?‰Û•MÜú?ïãCBÓG.?aË|Á)º«?l¼½,¸Ðq?aË|Á)º¦4FGL J1606.2+1346?¯¾ÓdÚå2@Eac^t)žÀ;]™J¿@óÀ<¥äŸQi@"j‰¶¢"?ûG'Æ}¥?Íkè.R#?©ZÞB ?ß³ 9†^@ÌR(–Í¿ïíû@R«t?ïûA
r¿ÛÙÒ#£É?¬öoÞ_Fb¿é2ŸÅ,Å[?нw¤ý%AGNbllMG1 J160619+1345?ïýgðÐk?2›Ó.Ò»?4À||¨ô?2›Ó.Òò?ïý>™ ?T¤xPp²?6‡Û6ÿº?T¤xPp®?ï±­
t?'ý¥ÂŒ8Ï?ƒ"¼¢Ø¿D?'ý¥ÂŒ8È?ïåŽoùBv?a
Åk¿ln?jq½Šd?a
Åk¿lm4FGL J1606.3+5629?æ|vqƒh@Fbb#ᆘÀ;&,ºs.À<Îò`Û+@!"5Á­ßÍ?ûvmÊÞ¶?Æҙ•gÛ±?²;-}'¦?ếBŠ¿@}ã¾V¿ï¯IÏVêÈ?ïìá?J˜«¿à‡Ëp¬:†¿ÝɨÀ~	ñ¿Ã<òϕÔé¿ÞÌDý
,TAGNbll3FGL J1606.1+5630RBS 1558?ïþòt¬½?¯0€' ? ص4/d?¯0€'W?ïý®\Ø;ê?L¬©¼b:-?2> ¬^?L¬©¼b:?ïò°‰ryG?`Að¦u2?Zží
q{?`Að¦u/?ïñ•ä^ôž?PéW!âÜI?\Ô7BÇQ?PéW!âÜ[4FGL J1606.5+2717?ä…Ö£«<—@Gs¹8›RÀ:"¾³.–À<iÉØü…ø@
ÿ¸\}@¥Áƍ?¿)âýeÇ¿´{ç¾%ü$?ô05½Q.Ç@ÔL\$8¿Ô< A¿¿ç×ä'‹¿æ"[t›¿ã"8^kEH¿ç0=µm5¿å9̪hAGNfsrqB2 1604+27?ïû/$¤å?BÔ¼GmÖ,?CïCmlp6?BÔ¼GmÖ"?ïö¾mürÌ?vZ×¥?Rƒ$i—?vZ×¥?ïÞ5ú4ø?tD€¨Õ-
?pååƒñP?tD€¨Õ-	?ïÚ+ö܏™?a
©T)c?rê'¸3A?a
©T)j4FGL J1606.6+1324?Ü>PJ¦¾%@EB¹¡vÝ­À:â°"rÐÀ<OŠë€í@+^a_@'@ô	¢@1H?Ï,—Õõ?Ã,éØvN;?ò œÃÆ@RÐL^'~?í¥"à¿ÙSº|¾§¿æ¹þúFƒ¿âBH§µç¿ê$«°óR¿ïÿI¤ë‡AGNbcuNVSS J160654+131934?ïfõg:‡?«ÄÌ!ºä?"!S½O*?«ÄÌ!ºå?ïÚä6ÌØ«?…d™Ê
?rä™"ª½?…d™Ê
?îÙ"·UE?•Phnma?¢mԎʫ§?•Phnm`?îÓ°L+ö?†qÎéƨ¤?¢Èû=@Ä?†qÎéƨ£4FGL J1606.9+5919¿î¯Û5ºª@EÙßeUÅÀ;X)º
­hÀ=qÞ@‡qÎÏ[?üÔ¾¹
Ó'?Ò+ÖÝò¹ñ?̚Ž…ia?ò‹ºc=¼ú@
^<™8u½?ÙcqT2U¿íR-ÿ틉¿³:è‰@Ü¿ÝÊë€ìúj¿é",<žìÀ¿Î{ÅHIúAGNbll1RXS J160709.7+592115?ïý
^ÒÕ/?5\Ràãºa?7•	iV\?5\Ràãº^?ïý©2²ß?Q²>,çRñ?2¶oRi¶?Q²>,çR÷?ïhû}hY?‹«ñ´E¼P?'àžðRôÏ?‹«ñ´E¼L?ïú«Y'ËÞ?1oÜ~`T?ER™¸Ð‰Þ?1oÜ~`N4FGL J1607.0+1550¿Ýï"ž`›[@E³ã*cÇÀ8•Ü¡u0À;͇®µŠ'@{/bÄw@"mH÷Q?¢:ƒ<=¦‡?¼i€0M6@80yþÊ@g~igw³?ïÈtþ¯è¿Þî|µ]D¿äYÝâìпäZÿ**¿¿çp²Osڿ鿞EÐÄ©AGNbll3FGL J1607.0+15514C +15.54?àY¯fÚ¤"?ʸPC¬V?ßL¡2J·¼?ʸPC¬V?".Kçß´?"gÀZ%†[?ï^ Ã?"gÀZ%†[?è5Âàꙷ?°.Í~ý+?Ï(ô|U™&?°.Í~ý+?¡4ÔûT­!?'™ÿ+×O´?îì²°Jµ-?'™ÿ+×O´4FGL J1608.0+4949¿éò"@¦i[@G0dÜY2À;d»—cYÀ<ëëºÏ@Œ¨N"5ý@'<?ÓÞ>ɔ^?ڙ‡%"Ï8@8OLnmœ@ék'…?îü'"ø¿©˜ P`¿âôu
œ;¿é5ðè5 ¿ß²¢\¶º¿ïýÿ!]ÉAGNbcu87GB 160630.8+495728?ï÷U噎^?SIþd=ôË?QT4ÌãD©?SIþd=ôÃ?ïü±_¨—?T‰DZQŽ?:t»RØ?T‰DZQ?î"ôÈÎ?—ß[´Óaó?¦°¾"s?—ß[´Óað?ïÖùÃüo?d
p²œ;4?tƒúH€?d
p²œ;24FGL J1608.0-2038?Úñ(¼ý#¬@6'¬dwxÝÀ9㋘O¿À<hXÓ×@…€flÆ}@ž§b¯ø?¶‡a!œÌ™?vàé—çE}?Á>ìdl¼@õ+ÆWgÆ¿åù§4ƒ?¿âEB;å¿âsáxU|¿ÞuÇ,yÜ¿åOv_Ø­¬¿ÕqEiÃAGNbll3FGL J1607.9-2040NVSS J160756-203942?ïöô8€Å2?KKQéO}q?RŽþuœ!?KKQéO}ƒ?ïþ›
.-ð?E­ð¦j·?&O- ò?E­ð¦jÓ?ïö+¤ö[#?bvÙ!'ùû?S¨¶IºM?bvÙ!'ùù?ïò^*LÂ?K¼ÝÙ?[Có«f}û?K¼ÝÇ4FGL J1608.3+4012?ÞÍþâCú@GÊʁ˜ñÔÀ;‡³-¿UìÀ<î™
'¡/@'0ÉKó?û(¥U~Ž?àÒèÛ­e?ᚮÂu°Ü@Q¹eç»f@Yuƒ?ïئõ¢¯¿Ú´ÈÊÍ.¿â›W¿"Ç¿Ú"K©¢¿ïÿûÎBÓ¿ì—æpâÁ+AGNfsrqB2 1606+40?ïîIYRéU?oÈèy¸þ.?a¶¦­ª»?oÈèy¸þ)?ïùJXÅQ«?a[‰ªÎú?J֜ê¹U"?a[‰ªÏ?î+[ìÍ©?›¨Ñœu«J?­JF!3%d?›¨Ñœu«L?ï€P¤Ë\U?~Y6¨n[ ?ëÖÍ(ê±?~Y6¨n[4FGL J1608.7+1029¿àDÙlš4°@Dg7âÅ\–À9($}ÊXÀ;æÜ0@úñ£Eë@©æ~Nº?°¦3
9?Ä^DC{Õ¹@Ęވ¶ó@*
díj|¿Ë™à¦ÉWø¿ä«±^²<ÿ¿ç^Á÷†´»¿èÓØYÉ¿ë†Á½¥¿ðAGNfsrq3FGL J1608.6+10294C +10.45?ïöX¬ï|d?Lî¼viû?SN¦!8Ð?Lî¼viû+?ïúö¿f%?Yo'úCƟ?D%¾gmû?Yo'úCƤ?ïVd¦õÞõ?[wøu:?•3k!D!w?[wøu8?ï÷rn?@¾zî¤IÃ?QÏ#ãöI?@¾zî¤IÐ4FGL J1610.3-3958?ïÍqZY±@!îÐ,ӞÀ8û²êòÀ;hâ·Ý!@O=yÞo@rÓA[#?´&òH‡X?¸'­¼ç&•@| fèl@n'ÏùR?ïÿ1£æúu¿åaRàø}Ö¿çm͘¤§¿ç㺺{'q¿æ%ہp'õ¿ïýYÝl[AGNfsrq3FGL J1610.6-3956PMN J1610-3958?ïýÜ
åO?0D×Ü2;6?1—øՂµ?0D×Ü2;?ïÁ¸àY–?"#±œ2á{?#Ó4õV?"#±œ2áz?ïe^;e^%?øæÂ?"T8"T;b?øæº?î÷'sNá—?†kË£ÑË? ˆËæ¥?†kË£ÑË4FGL J1610.6+2414¿ïý4ä/ˆ¯@F©A(¿<À:ŠŽ›8Ö
À<W[ìà³@ýI¤¹³@@ëGâàí?¹Áµ¢®Á¿¶[¬¤
eï?û=L¬€üë@5ƒo‹©¿áÌ=]º¿ç+{؃¿ë"9`÷ã¿Óe="[¿å£ÚЛŽf¿ÔÎ9´V´BAGNfsrqB2 1608+24?ïø›ÿ1â?UàX™?M:x+?UàX©?ïûžsôÉÞ?i̖çñáñ?A†0,؈?i̖çñáê?ïŸOf?‡ôÛ)³Üd?ˆ88l&{H?‡ôÛ)³Ü^?ïäò}\›‡?_5\R ?k
'£dxš?_5\R¡4FGL J1610.7-6648?î}OÇ`À&EÌBcQßÀ80äÅçÖ>À;]C¢ìÿr@m‰'8Ìû?ùÑb§•?£rRØ¿õ?¼fý4ÑC@¯Â¼¨'[@Ëïž]ù…?ïýÆ¿Âx5¿Ë‰ g¿¿ÓPÛ$Sql¿ÒjCÒ ¿ÚÒTჾ¿Þ(ƒÕ,ÃAGNbll3FGL J1610.8-6649PMN J1610-6649?ïî£éÚö?jÅhã×[?a\%	æ½?jÅhã×Y?ïd–+9È"?¯†µ=?"m:˜ÆûÁ?¯†µ=?ïNrkjá~?"NÀçòMã?–1²'£Ð?"NÀçòMâ?íÐké'0	?È[­…Ø?±| ¶Æ¼?È[­…Ø4FGL J1612.2+2828¿ï
zICn@FóI{t¥À;j€G¸ü5À<É~#òM@ˆ0,–?þ6§¬Óª?Ó6^á·Àv?Æô$j Ü?òÍ…/?ÿz·^P˜I?çÿMR8¿äwý''i¿ÑE†\{&¿ãþœÞGžz¿Ö`ŒÝž5¿ïÿ®©ÌAGNbcuTXS 1610+285?ïô™ðïäz?TCo¸¼?VÌ 7	2?TCo¸±?ïû«Ü!)Ö?VG]½à?AP{X£_?VG]½à	?ïƒ\Ew9À?‰o ìm3?(î¢1Û?‰o ìm6?ï›øÝÈBÓ?v} u·<'?‰ȍïJü?v} u·<*4FGL J1612.4-3100?î³DÁf'õ@-P¯>FŒ¬À9a³õerKÀ;ÐôƒÊû;@µÉ¢ö»?ÿiðÿ±üg?²ÿÂÊí?Ár^—:@¤[^Ëgr@7ºC³3?ï÷T?NÛ¿Û%î;²]¶¿ßö"ºÝa¿ÛüÚ\¿çÄqê('f¿å	BsíãAGNbll3FGL J1612.4-3100NVSS J161219-305937?ïûEç?E:†‰¬Î?Bë㏀a-?E:†‰¬Î?ïñ¦
.±"?tÊõš¸Ñ~?\³å¢œÚ1?tÊõš¸Ñ{?ó=î;?‡š7§žþ?‡ŸC0"q'?‡š7§žü?ïäÍFÒüÈ?Ti6KUu?k2¹-8?Ti6KUs4FGL J1612.4-0554?ï¶U´ë@?C«CIIÀ:pHD<oóÀ;÷žXE;s@y5ËéÍä@­"'±È?Æ=vƒ? ŒÂ_zRÆ?Õ\cÞл@5H
æš?ïþ_ìÏ¡"¿Ö†—^Uö­¿í´4 ½¿Ó#>ÿP3¿á‡£,ÀRk¿ïÿý{ÁA~AGNbllNVSS J161228-055752?ïüérpJU?Eb0	"X?8´l}­P5?Eb0	"R?ïþH‡\\$?Env£Wv?+wŠ:=ÍÈ?Env£W]?ïg8Z$ù?Œ#¢@
Ý?"ô¾›a?Œ#¢@
Ú?ïðEùw™å?Pq^–|€?_t
Ì5O?Pq^–|l4FGL J1613.3-1907¿ïÆ	´ö @6®g¥*ÇTÀ:°Ä±uXrÀ<‰X=@ fÔÜeÇ@™×ºf˜»?Éé'¶Ó;Q?¹hìÓ}k?Æ£ÌùBv@ºØØãÁ?ÒO.¦Üx;¿æ38q`•l¿à㠀þî¿Ùµ
¸A%¿ìÀÊ*Ü?Ó㻹ÿìAGNbcu2MASS J16132720-1908364?ïéU6±Z?eo<¨ø?fñªÉN¦\?eo<¨ø?ïýÛ¶3ò"?JÊí.¥?1"N`nç²?JÊí. ?ïZ­=Õ?z'ôZq?"ªX]½e{?z'ôZo?ïçÃ\ÙºŠ?Zˆ?ìVØß?h<£&Ev~?Zˆ?ìVØÓ4FGL J1613.5-4225?È(Í9Üd@H)ŒÁDÀ:P#tƒÀ;'I:µL@czðáÿå@€c?jy?Ñͤãú'?·aÓȌv?ìÿMB}þÞ@ˆád3†?¿ïôµ´'S,?ïÿÚáb†¿ìõ¦n"¿Ù±ÙŒÂÇ¿æú"ˆ¸¡¿ÚŸ)ÜvAGNbcu3FGL J1613.4-4222PMN J1613-4225?益¶!–?Œpj«3×h?…Ú}÷š]?Œpj«3×h?ï$,¡˜Q?´`äms?›zkÌüÕý?´`ämr?ël¿A?±¸4ŸùX?ÂOﱶù?±¸4ŸùW?ïnõ
p?‹–ʪN?'!\ŽR?‹–ʪN4FGL J1613.6+3411?ÃNJ±%>ó@G0Nø‹—xÀ9*E†òÍèÀ<DÊPñŠ@£KëW@Y䒼/Ç?¦»®—WŸú?Ÿ–k;ã0?óFÌ¢Ûa»@Ñ´ì–¿Îú"€'ÇE¿áýÔ þþ"¿æbE'Ë¿ç~b †ˆE¿à'Tჾ¿ïÿ‡¿ÒhmAGNfsrq3FGL J1613.8+3410OS 319?ïý³C	˜V?2¼‡µt€ð?2eç³=X"?2¼‡µt€Þ?ïüŠY2'z?Q½¨6
¥Û?;­6nÄ+§?Q½¨6
¥à?ï吉4½$?p&/˜a?jovËBÛ?p&/˜g?ïúyʊñ?;¢Å0ߕ?FÕÔ;ѧ?;¢Å0ß¾4FGL J1614.8-0850¿ám×*†›6@=É>¢ÒþÀ;7x"væÀ<_"\h¶£@"җ֜Y?ý+G&/>²?ÆeXŸSl念)f€½¨?𗐪ݎ¼@~I‰¶Í‡¿æœ"¤?¿ìGðI´¿×ôƻ栈¿éùqÁ
{꿳Ce/"§ð?×â•@ÄkTAGNbcu1RXS J161443.4-085130?ïÿlx)Á?>{.%»?púÇÜí7?>{.% ?ïþÎá,Î?Ex"º‡ºy?.Sí3!»?Ex"º‡ºX?ïæYúaZ?r
zẠ©?i¦ž¥õ®?r
zẠ´?ïúöíI¾?BEüg.¿C?D'ðJÙp?BEüg.¿>4FGL J1615.6+2130?ïò
Ã(XM@E¸óË>WTÀ9ù9&BÀ<?k@Àºp@˜÷-žsÉ@ëÏkn
?¸aöKKX?¡¶m嶩?áMp€ñ'@\"òB¨¿Ã"ïCDMb¿è8ÁצE¿ëhÎUcä¿ÛÅ0@'/¿êÃJ¢»K¿ïáñ¿Ë]AGNbcuSDSS J161531.09+213011.0?ïü#QmØ?<AÊ9·©-?;åt'L5?<AÊ9·©$?ïýÐØëB}?Lӄ•8h?1y8¥ìñ?Lӄ•8c?ïË°¤XiG?€DÖTˆà?z'­ÓË]?€DÖTˆà?ïø–¿ˆKô??âxZf?M¥ÞÐ3y??âxZl4FGL J1615.6+4712?¤g~
¯iß@FÎãK"SÀ:C{À<‡)éÞU‹@å5oùb,@GÇ$_¾?µî@dô÷8?¨f*ßÛ%?òŠFu/W@Ÿ´Ú'³ ?ëw¨¾$¾P¿Ñ´]¸½¿åMI"žˆ¿ßéþ Õ®¿ã&óõ/Âe¿æE£þwiÄAGNfsrq3FGL J1615.8+4712B3 1614+473?ï÷€ ⱒ?D1]Æí?Pÿ¾:œÚ?D1]Æû?ïû–N+?Vøq˜4&¿?A¦ÇŸQÆC?Vøq˜4&¹?ïëü¬Bæ?pQ
><.?dâS½?pQ
><$?ïÉáÏls[?ctPDñµæ?{IÆQ³?ctPDñµà4FGL J1616.6+4630¿êp¯NÀ@Fœ¢ß"yÀ:ØÐi9~À<-\6@øÓËCµ·@±PÚãæÅ?ÅM-šÂäl?»þÇƨ›j?ñoxäl-@CP¿Ê^ªïj\¿åƒ]b[¿Ä¿éR,†pÈ¿ì2àÈ,T¿ïùÕyC¸¼?ïîê>!βAGNfsrq3FGL J1616.4+4631MG4 J161600+4632?ïþ´äŠP@?%Mê <7?$±·Zü	ä?%Mê ;õ?ïýhÚ*ŠR?KÚS¬q€?4¹.«­eû?KÚS¬q€?ïå(tK?pC
´ä?j×oዴ×?pC
´á?ïôÃÿ@³:?IÛÕî]ø‰?Vx~™‹#?IÛÕî]ø"4FGL J1616.7+3327¿çS
b,Ã@FÖÄ`퀡À;ô/eƒÀ<¯'ÎÉý@g(<	E¤@:#|ÜÊq?ÒÛ<'¦?̍À‡ïø÷?øì#>Éik@vþöj«?ºÂÊ?~Æ¿é"i†¬W¿·™y¹)'¿á`àpÀ¿æëg@ò¹¿ïøUFƒrAGNbllNVSS J161633+333043?ïï"Ӗ*?]Ø«lrç.?`kï,iÖe?]Ø«lrç2?ïú@oåÊÌ?s|̪¬ÂŒ?Fþ@hÔÆ?s|̪¬ÂŽ?ïž[S,Ìk?‡|äõîŽh?ˆi+4Ìå]?‡|äõîŽj?ï¸5"ÇÈ?fƒ`ÖCS?ò›
ø¦?fƒ`ÖCU4FGL J1616.7+4107¿åగYˆ@Fúù3]$žÀ;îgQGñÀ<ÝÌúïõÇ@p@'Òë@Rºà;>š?ÇFBšvØ?ÆðÀU?üª«õ¼°@I+®Ús~¿æÿb`ÈAο³ï(nß¿æ''àðp@¿ãk¥Õçþ¿êžJ''¿ïÿý¡UûŠAGNbll3FGL J1616.8+4111B3 1615+412?ï8'ãjSï?—i·G?«e?˜í£'µ'9?—i·G?«f?ïï	ƒ"ó?l+VÈë˜?`ö|kèÍ?l+VÈë–?î)®Sê§]?ú_µˆGÎ?­eÁUŠH?ú_µˆGÒ?îö×¢\P?ˆ~ñIFj? '…Ú:þg?ˆ~ñIFl4FGL J1617.2-2535?د€C´Êg@1£Ï_ND1À:a-ñªÓÀ;Ñ}‹Q@ïՃ)Á@™ð^¢LÇ?Ð;¹eç»?×ÑË9NÖ'@¢þ'Q~x@ü¹"`ʛ?î´º𠏿ÑW³°œž¿áÌþ ÚU¡¿éÒI
{¿ël‡þ¼'¿ïÿþÐñAGNbcu3FGL J1617.3-2519PMN J1617-2537?Ú¼–p)?•?ÇÎ(Çöň?â¡´Çë`6?ÇÎ(Çöň?఍H¥®?ѳ= H§?ßøžån´£?ѳ= H§?Ú]c¥"¼?·³,›n6³?âÑNs-=¢?·³,›n6²?à
`_c
?°(uáî?ßå?A9Ïå?°(uáî4FGL J1617.3-1513?ääȼ·@8†Šar
À;Dèg]À<¤Ú/­m@ t‡t~8?ûÞþ'¸«®?ÒÃöúȳŽ?ã$ì^¥«@
ü«>݋a@b§¿÷ý?îA$øÝÌÏ¿åwÿ ´•ô¿Ã"žWïU8¿ÑM²¥Ú¼¿ä·Z¿êU¿ïÿl\I¬òAGNbcuNVSS J161713-151058?ìáy¸ôás?³O¸*7!V?¸ô28Xô`?³O¸*7!V?Üù_Fa*?Ô÷²ôvØ?áòP\Ïl?Ô÷²ôvØ?è0jÜPb?·i'pó|x?ÍË>TŽ¾s?·i'pó|y?Üö8P?¸×¥—"¡—?áòã¸tX?¸×¥—"¡—4FGL J1617.3-5849?￱8£ÇÀ¶R7yÀ9>Ì?ß À;"ˆ9@"שÇÁ@ŸÜ>Y×ã?µM16-äj?Î;y}ÅR°@Èa-A'@NÔ¤\–?ïÿ¼®q—ó¿ãJ;ÝüŸù¿æ^:é
5¿æ2qôÆ¿í"t¡'Œ_¿ïýÍ ²<©AGNfsrq3FGL J1617.4-5846MRC 1613-586?¯¸ä?†&¢Ëqã<?‡>ÝÔÆç?†&¢Ëqã<?ïê ðO?v܉ŽXÕ?e_°ÿû?v܉ŽXÙ?èGî̼è?°'ü8Å¡?ÎàDÍÄb?°'ü8Å¡?îüJ/"ì?Š
¨€Ï—? ;]±>X?Š
¨€Ï—4FGL J1617.9-7718?ç²î"\À2ÞM;òõVÀ8tvÔr³|À;²/,=u¬@‹Rùw$Ð@ƒ'?	*K?¡.—3M_?¼¸ÈúÃ@À‡Þ†2µ@©Ö¨˜»¿ÖýCãÅÝ¿ä…dXo,ß¿è™Ì$0`ñ¿èH*;<ìð¿èS½í5øà¿ïþRúÉAGNfsrq3FGL J1617.7-7717PKS 1610-77?ïþêkKZŸ?rx꿔/?!YKJVg?rx꿓ê?ï÷MÍѨ?c1HÊ‹?Qdd]±‹?c1HÊ€?ï§H¸ÕŒX?…ÎÔŸ•¬?†-ÑʜéÏ?…ÎÔŸ•ª?ï÷ÓÌ-aì?@sTo÷³?PXg¥<'µ?@sTo÷«4FGL J1618.0+5139¿¿ú3ÊYòÛ@F8AVâeÀ:Žf$ø
À<ž0´Ó±Ã@Ua÷ÁÃ@†6Œs?˦>m£ò?Ìd6÷—&?ýñ¹KÈË@µ"Üž¿áÊ~ŸBP¿âÐ{÷È¿ç=xÁ‡Ê9¿í8Æ_ö4пåF/ßÁœ¿ïöØmAGNfsrq3FGL J1617.8+5137TXS 1616+517?ïý)žQ\C?9"Řð¨?6³
uãV?9"Řðæ?ïýLò£.€?PÛì	Ã?5˜jæ‹ô'?PÛì	Ã?ï\Ò½"ß?•0''¹H}?ôe¨M"]?•0''¹H|?ïþ;"Iy‡?öžÒ@Ö§?,FËhg˜?öžÒ@׊4FGL J1618.8+0620?á¡ä@BQAAé¯\À;5¢é¤sèÀ<šè¯bk@*s6›f?ý™yƒyœ¤?×3Úé%?Ô¹‹|uqq?ûŠ'5Îï@ëyÙ	ññ?ï¶`^åh¥¿ï)BUæ?í1Ý'ãƒ¿àtž7ŽÇ¿è÷ôÎs•ú¿â.ó2'#"AGNbllRX J1618.4+0623?ïè§ÖöÔ/?dˆT"Òƒ4?gX)	+Ðß?dˆT"Òƒ/?ïû5H®?\2^®!h?Aû+êÝL§?\2^®!j?ï,xªvëß?'3zYT?špê±""?'3zYT?ÆÆ¡³?zÛ
 FÄ?ˆœNW" ?zÛ
 FÁ4FGL J1619.0+7536¿ä{¼ñ"@A¨ôàM/À:˜NHboaÀ<Ç>óZÖ@7*Èü@:dÜY?ÁØÍ÷o7Æ?ÛŽd9îí?ÝGåœÒ^1@D qúï¿Ò3 ~O¼+¿æÌè`§	Å¿âߟb[j¿Úa(	3…¿ÕÙôÌ.A¿ïÿÿ&¦³AGNbcu3FGL J1619.1+75386C B162034.5+754454?ïù¸Xà@¶?H1dÿ?Iœ~ý)Å?H1dÿ?ïý¤,&p?JSøv½?2ޞό‹"?JSøv¦?ïçY¼®Ÿ?sûÔ	"öU?h¦üCQa?sûÔ	"öL?ïè"þ›?TŸ $Nqé?gÝôdå?TŸ $Nqî4FGL J1619.0-8346?í¼ÖVJÀ71qâ›k+À:õ6¥®zÒÀ<.Ï d$@¸½Mþ»‡@ú?¤Z½¼?ÉõMõVXÒ?¶s€wµ?éؽf'|F@,9í±?ã£Æ
•ê¸¿Ú•yyh¢¿à»²]µ½½¿èA•\¿æ;Þ§j¾¿Ì9\-AGNbllPKS 1608-83?ïì+ÉK%?bCú"{ç?cÔ6ü´Ûå?bCú"{æ?ïòw¨¶m?v5ïô¦
?[Ù®"'H?v5ïô¦?ïv=~LC{?‹¯ãú•­?'8P6wš?‹¯ãú•­?ï¯Æ}œ?@?mi?:^?"`˜ð0"?mi?:^4FGL J1619.6+5536¿í'PÆö*q@E¡Þ?»×²À:†—¨'ÑÖÀ<³¯' Wú@5ÈRi¯F@õÀ[¥BD?Á7;ÀöTÛ?À¹‹§h6?ûIKRä©b?ûÜP§¿¶abEšh÷¿ä‰»j¤¹ˆ¿åê™ÑͽŽ¿æ]¤öÄíÛ¿éÜ5 uÖÇ¿ïý?ÔVYAGNbll87GB 161814.7+554307?î—a¥4ö?£"jüéµK?¦‰å¬°ž)?£"jüéµK?íԞž'ùÜ?ºhUt'óZ?±[À1$?ºhUt'óZ?r?—‹ñ?ËÓ¾?¥/>Èè?—‹ñ?ËÓ¹?釥doÉ?¯žŽQÙêŸ?Éã­jn@Ý?¯žŽQÙêž4FGL J1621.7-1103¿ïmJ(Q	@:RÖËSP	À9ƓX6ø»À;ò­×>?×@‰s,Û*@ÐÈb?Âz	2®?ÊÕÊw]¼@7E«I@r 
´®?ïƒ=lr"¿Õh'{Mz¿äœ»sG ¿çÝ]Ó6¿ïóüQօ¿ï¢æÿþÓZAGNbcuPMN J1621-1101?ï…ø^N^?‡"¶a{R?Ž¿èlhG?‡"¶a{R?ïû»­D†›?T´aќzˆ?AJíå"3?T´aќzˆ?ë3x›ætó?ªBi—»½ž?Ã2f,9?ªBi—»½ž?ïÏÔT2H±?dѓ
h¨?xÕæÛ§v?dѓ
h¨4FGL J1623.4+0858¿Á½É+TK@BpJb#á‡À;a)ÄÀ<Œ«Ü'<®@ \<
<ç@V/Äé©|?È0§$G¿Qq±‰@4CºêÍ?ïü–ô£«k¿Ô톀¸!D¿ç|^?¦^#¿â?ü¥¬¨?±yÃeoñU¿ïÿÿ)@k*AGNbcuSDSS J162330.56+085724.5?ïýVprk?BTgfC ?5L|l§>Î?BTgfC?ïþ0"7F?EÃ_¡?,ö¾l‹')?EÃ_¬?ïá~jCw?t¨7ªÍc?n•ø¼‡U?t¨7ªÍs?ïû>ZÄ÷?5||MÈ?C"ì#"P?5||M4FGL J1623.6+5743?ï€Êžõ@EÅXdE$À;÷GʚÀ<ÝxC½@b*"y@ca	/T?ÃWSùÒ>|?"ãpäTäð?Ñóêî?ò*}'Þ?ïèÙ¨}b+¿ãC''%ο؉ }8é¿ãã'àp¿ë|'Biñ?ÇÈ?Il¶AGNfsrqTXS 1623+578?ïç7󃀼?hmê$T'?hÈ|D
?hmê$T%?î·ÖvDí7?¶yÝ.?¤'˜›±,‰?¶yÝ.?ïÏ2?"*-ÔkÙ??Oß&¼?"*-ÔkÙ?ì˜"=R\?¥ª)Ì´?»>î]m,?¥ª)̵4FGL J1624.6+5651?ɹ1Eclv@E!©T!ÀDÀ:΢Ç?ÅÀ<Åð®{©@Qœ«qÞ?@	A=?½¼ËLïò¿FÚ«´XŸš@cý/ìð¿ï†'Ìͤ?ïŸà¥Ç¥F¿è6¯¿uÌ5¿ßQƒòÖL¿à 4óý">¿â[7(‹9…AGNbll3FGL J1625.0+5651SBS 1623+569?ïñ—Ÿ,ï¤?Z¤ÉÜ)D'?\ÐÁ¦ ¶T?Z¤ÉÜ)D?ïüh¾–2Ö?VUX`jÿ?<ºNiIß?VUX`k?ï߹Ʉ¡?rDÝFXÛ?p#=þ¯»?rDÝFXÏ?ïårgk÷?[mBò`-?j˜"ûÑ?[mBò`.4FGL J1624.9-4210?y".@1ßv½À9°\'¹À;2{"¶
n@é¢[	;@,üœ?Џ½ei?äý®l@Zw¿á?þÌL&t3?ïê4†ðIª¿Þ{?[µˆc¿èß6üìOI¿ìxToÃÝ:¿ïÿþó…õ?è–ý]
wAGNbcuAT20G J162458-420657?ÇIm¬èŽP?Å_9x2±5?ê-¤"ÅÜk?Å_9x2±4?¹Â4Ëüb?ȵ÷Žû;?ìǹf€lT?ȵ÷Žû;?ӌàN+ý:?·? 2ÌJ6?æ9Øêc?·? 2ÌJ6?Ö?‹S§?ƒˆùs¸î?ïyN§=c?ƒˆùs¸î4FGL J1625.2-3600?»")¦5‡@"|ڐî¢À9ô
 yóÀ;"Œ"ÎX¾@4ìƽ>@Ÿ¢È…?ÉQÄð_y?˛?áíEh@¤åýö;?ürµ"¡ã?ïþ{eÑëð¿Ú1/"‡•¿é³iï‡â¸¿çØ-Þµ'ƒ¿â¤C@Çp¿ïþ
ýŠúAGNbcuNVSS J162522-355452?èmzIi?ÈéŸÑP	?ÍÊKÒÚY?ÈéŸÑP	?༅•û³}?ÑÖAG/¥?ކôÔ™?ÑÖAG/¥?ãTѧp?½TŒL/?ÙV\±Ûø?½TŒL0?àôéU€Ä|?¶ˆgîOŠ§?Þ-Tþw?¶ˆgîOŠ§4FGL J1625.7-2527?îÄ*©ãZ @0PÙÆ°SÀ7ÇϯÖÀ:ñq¤ˆ
%@JIOTQ@_3¡íûñ? :)­?Áªàú®‡@ n
ˆ~¿#@ —Œùù¿Ê"¸ç' ×¿áXß_vˆ¿äy`¿'F¿å(Ø0®µ¿éÜ°|¿é¹ÅÞñèeAGNfsrq3FGL J1625.7-2527PKS 1622-253?ï53¹×‡?¯ã¬œó~ç?™YˆÅÚ?¯ã¬œó~ç?ï§æ–œuV?£l'ê*Í?†ZXâª&?£l'ê*Í?íõA,îª?ŸÛ ®â½×?°U÷N˜Š¾?ŸÛ ®â½×?ïï0slP??V
PQÑe?`ό"¯ÁV?V
PQÑq4FGL J1625.7+4134¿ï¬òWwH@F ±Ù+€À9Ê"
qÀ<qºnü7@‹#IWƒ@l¼Á¼ÎR?¶¨åf÷…Þ?ÄÍï»õå@êiæM§S@bÜʵ›¿ß¬;W¿ãÜâąֿæQ%AX¿çˤ® '¿ïÿ°7ßj¿Ð¸âÓõ5AGNfsrq3FGL J1625.9+41254C +41.32?ïíÂ8²…X?dÌ:Ûsì"?b=ÇMz§(?dÌ:Ûsì%?ïøODóÓ?e$¤ì"'ô?NÂïô0¯•?e$¤ì"'ô?ï,G{€?"÷#À]Ì?œšw‡¯ý?"÷#À]Ì?ïÏÕt5_S?gñçîw?xEåPUä?gñçîw4FGL J1626.0-2950¿ïÖ=Ln-"@*§ïZ–N‹À7ö¿Ñ;ÇVÀ;O«›úœê@L;kæÙ@§"ÁÄO? æ……x3?Á<'§º™™@Øņ‡n@EŒê߇e¿È«]üµr¾¿ãS–JYÀf¿ç¥mB"º?¿èÀ;Yrb¿éüc'í"Ó¿áV[áþ`AGNFSRQ3FGL J1626.0-2951PKS B1622-297?ïë xF'Ô?c6&Ȉ°v?d_‡¹m+ø?c6&Ȉ°u?ïÐjÿ‹R²?¡gO{ÂÀ?wʀ:V§j?¡gO{ÂÀŽ?ï
4Ùl?˜"R°c¼R?žYdݲ|–?˜"R°c¼U?ïàÛ4ù[é?_º¤2ÖÚÀ?o$ˤÔ?_º¤2ÖÚ¼4FGL J1626.3+3514?í±ïÎk«v@Eñ&|k‹iÀ:ý|ªu‰ðÀ<±vö×bR@!)æڕl?öÀ;ú'¾?Ð$þÝ@7~?ÐR9¦j@qŸÝ€y7?þ½ ŸrK¢?ïm­íät‰¿ëU.enâ¿Êj^¼#¿Ê'dÜx'a¿ÞŸxkK¨u¿á´¶á(#‹AGNbll3FGL J1626.1+3512RGB J1626+352?ïùg
°t—?DS"É\k,?JcÕ>-§Î?DS"É\k?ïår—U*'?¼Š;AH?jhªÕØ­?¼Š;AH?ï²åzö,?€ÞwM§$?ƒF¡Btü?€ÞwM§$?0'2`?'>bÇ-À"?¥Æ÷ÜÚ?'>bÇ-À"4FGL J1626.4+1820¿ï'd«†Â@DãC0×8À:Œ"¦£mÀ<H'sg@u–Eý`@ÞûB0&?ÂhÁ_†M?ÏáÕ§?ÔM¬[==@ôB‡¿å;¹^Û؃¿Õ~àEO•j¿ì
c›°Ë¿áš«n®4¿à†FÁ—"¿èP%1€¬AGNbcu87GB 162358.1+182615?ïç"ݎsŠ?pRa£u©x?hÝ"qŒv?pRa£u©y?ïýø1x?Nwþh¤1ð?7?(>t;©?Nwþh¤1ø?ïcÖµ9?/èø —Š?"%0	Xñ?/èø —'?ïëÔ3jv?U"˜þŸX?d+Ìú•ˆg?U"˜þŸX4FGL J1626.6-7639?ïÁ±7Ô¡À2͇+À:Ba¤`À<Rmý3œå@ /ù€_
ý@LÓi©?·b>
¬»à?^ê8§în? ˜‡Üéá—@	xš¶O1ì?×»©äÀ^¿ÊDAùI­¿ãqøjà¿ßŽÞ	àÿ¿àúÓOÍ¿Þž6œLÒAGNbll3FGL J1626.4-7640PKS 1619-765?ïýzu»n?0t$:t¸?4,WÚ$…ä?0t$:tÄ?ïþúì
¯?;Ž2ôU? Q?_u"?;Ž2ô•?ïó¦.㱒?fþr®ù?X³¢8œÞ£?fþr¯?ïùüxj]ë?8É÷¶Lë?HVˆTQ?8É÷¶M4FGL J1626.8+4337?ë¤y(AÜ@EÿO?Ù3ãÀ:ÏÀXJCñÀ<Š¬®IT@ÀjS†@g@€ù?ÈQ:€Y'?²²"Ç!è?ã±2!»;«@îOá¿£?ï¿}X›M¿êB€x`cî¿ê×¹Z)AB¿à£Ò¢Ï£A¿ïþQ€ž¡¿Ï•½ÁìôàAGNfsrqMG4 J162551+4346?ïôÈøĨ/?rÌù†ñTú?Vnv¯¢Ç?rÌù†ñTû?ïÑ,­á('?'sÙ%~
?wi©k·D?'sÙ%~
?ïÊH_VDÜ?w}N­IA?zÛÐTݑ´?w}N­I<?ﴃ®›Fà?u콑š?'ßY.HU?u콑›4FGL J1627.3+3148¿ÛK4æ\•]@EŸå\ËOÀ;
ÿ'E7À<ªmà®+!@ ¨7F=Q?÷º›<1·?Ò×Î]›'–?Ò¹C£Bå®?ôJ…) z@ò‰§ß®¿å—O§Ýÿû¿ÝÔëŸuѓ¿äàNjDlA?¶g¡	$—¿à
¨à"Í¿å¹êqùA AGNbllNVSS J162712+314954?ï÷'‹|ÿ?G1þeM?PÜéÕ?G1þeD?ïý'eG?K	Pû‹p3?3ì×[Í;?K	Pû‹pB?ïÁ&íFÂ?€VÆÓí¨?rl‰\ža?€VÆÓí©?ïîb¥V—z?PžbÆ¥œ ?aZ©h‡±?PžbÆ¥œ¤4FGL J1627.3+4758?æ,nÿ—¢0@EƤ~Ïé¸À:вýî­ÈÀ<™M߆ã´@Ÿ…@ò
¤@Ú`üšò?Ê0HÔÛd?ÏYÌ9©ïÓ@¿<pɖ·@"¹D8¿¿å塄õs¿àÝ6aé¿æbEÚÕ¤¿ëd¯­Uk¿ïð¨ÿ¾Ç¿é	lLþAGNbcuMG4 J162750+4802?ï'ä-}îØ?'&Slêå?‹Fô "J?'&Slêå?ïäåäo‹?ª΁ñ{?ƒcCrž?ª΁ñ{?ìÛ£m•ˆ?¥TÙ[˜Ž?¹"ç"SÂ?¥TÙ[˜Ž?ìúÕɚÅö?¡hþ¹Á?¸)Q³)ÐJ?¡hþ¹Á4FGL J1627.4-3301?ßßÃÂP@%ëßm¹@ÿÀ9ÎÌ¿`ÓÀ;Ž1á#›æ@÷âzÞîb@BVÃ[?Ä¿4žBJÓ?Æ«:ÖÀ–‰@ÒÌ:֕£?öÙ6Âß¹?á¡èˆ6?ïüÀآĿê´k¬÷Dp¿âi`Kš2F¿ð?ïÝüÀ/…AGNbcu1RXS J162725.1-330322?äo"¸yql?Ϩ¹dqG?× Ö
(?Ϩ¹dqF?×Ð3þ•5?Ôbü¡ÃƒÉ?äæµ{å?Ôbü¡ÃƒÉ?ãÁò'iM?¼tèÿÎ+?Ùî|Û-f?¼tèÿÎ*?ÏÈ
¸J¿?º4Uÿ¦½L?è
úýQíP?º4Uÿ¦½L4FGL J1627.7+0251?Ðöu5â@@{ñA [ÀÀ:" ‰ƒœÀ<o§yV-3@F‡"^qO?ýŽö¨hi?Îs€?ÖY¾?Ò"¿µî?ÿäùdŒW@	âe£û
¿å	%B°¿æ…ZýýqZ¿Ó77dENê¿á­š'w¾þ¿äÞ><ü‹¿ïìüLíAGNbcu3FGL J1628.1+0254CLASS J1627+0251?ï÷²ˆí?R鉞Ýø7?Pšî%ÑÚ#?R鉞Ýø0?ïýçhA\6?FÔz™fÑ5?0ĽõHM?FÔz™fÑK?ïå.	ó?">"¨þ­?_Ú>ÁÀ?">"¨þ­?ïë5àwÒý?P9¡BùÛ?dʈ-Ê?P9¡BùÞ4FGL J1628.3-3343?é0Ζè§f@$±·|¯ÞÀ:ê#èùÀ;âo¼h@ Y¶Âs@Õþ¤¶-N?¾«>‡¥%i?';|¾þ"+?ÖÊû>ÊÁ@.d,$v?ïþÙú²¹%¿ëb†÷¿â‡k>gnÏ¿Þ1œDÄ«¿áP·b­IO¿ÓW<½J£½AGNbcu3FGL J1628.1-3344NVSS J162819-334342?ïè›jÎ7^?f]غ's?gd•1È¡ª?f]غ'n?ï÷³÷œŠ?hõ*"vŠ?P˜ÎÆìp?hõ*"vŒ?•†ˆÃ?Œ4<'&Â?ŒÑšž]Ï#?Œ4<'&Â
?ï·&$ãܨ?mÍB _¾u?'6vÇÕÈ?mÍB _¾s4FGL J1628.6+7706¿î#Р2šï@A
[–(ËÑÀ9¤š~›çÀ<,žZÉz2@H¼áGX.?ÿS‡œAÇ?¬ß¾¥Ð?·mÅÖ8†Y@
Ý®ˆ*Ü@…í
´ôi?ãþC›`C¿×û=j¿à8@¹-³—¿á­ýžü¯é¿ä"q`¿åò"šCäAGNbll3FGL J1628.2+77036C B163030.4+771303?ïþuŸîw7? ŒóøO©?(¦Œ'4? ŒóøOª?ïúބÔm?]Œ¦ÃÄV?D…ïÀ®J?]Œ¦ÃÄV?ï²±h?'³bzè?ƒSº}>&?'³bzë?ïþï
ò†ª?Pl0Ô?! וu2?Pl0`4FGL J1628.8-6149?ãÖß·7À"a'ÚÀ9Z귙^áÀ;³ÙésÍ@Ÿ¸7"kÝ@Æ[ê¡õ?µ›ƒ~¥!?Ϫw¢Î́@"ƃÝ@ã&q÷?Íî´(;2†¿ãf…·æ¿é|¢èÍ´¿èÝíPÐÒì¿ì̦×o½þ¿ïý9Fr«AGNfsrq2FGL J1629.6-6141LQAC 247-061?ï×h§Ç?¯Xq¾7ê?œÍåë?¯Xq¾7ì?ïÁ1}¦ö?¢d¨ò4Áµ?gAx,"ý?¢d¨ò4Áµ?ëÀ(qÁϽ?«ùxԀ?Àÿ^8øÁ?«ùxԀ?î  &6e?öž
çéØ?¥õýœ™®Â?öž
çéÙ4FGL J1630.6+8234¿írUB¹Òš@?:kÆ!·áÀ9
¸ª*À<&VÁ­´Ú@Îæcæ"@²>¬
:?¥ž»AŠ?¶Ì`@\'{@%äêÐÄ?ýTâƒBj¿±yƒÿæ¿ß^謿ä¥/š!~Ö¿æB• Ž¿êÛíÒt¿ç
'Kº"AGNrdg3FGL J1630.6+8232NGC 6251?æ÷wz'Xm?ÅÛ)¯פ?Ò
ûO'?ÅÛ)¯פ?Å;J©…ˆÔ?ÌnˆÍPl?ê±-UžË?ÌnˆÍPl?æ,¸&cQM?±E?'?Ó¦³9]g?±E?'?И{‹Ïô?¶DÑÔ»8ª?ç³Â:t?¶DÑÔ»8ª4FGL J1630.7+5221?Òd‹?)ސ@E2\'ÑN<À96Jbú¡À<Ãõ¶7@G¶¶_øä?ÿ%"Ùîô??¨ø%
?Ž?¯Tkì @Oäë8@	l,¨T¿ÔzÁWÁ¿ÞÚÙÕÊ¿á*p·"@¿Þµ6˅…¿áÝù ?{¿æO6WªâAGNbll3FGL J1630.7+5222TXS 1629+524?ïüÉÉ»ã?17~ͯ¢:?9±² ç­(?17~ͯ¢:?ïù	ùúa?aaÏC_¤ã?KÛ¸}T?aaÏC_¤ä?ïâ,id?pvü‹á?mӖñ›üO?pvü‹Ü?ï«!#v¨¾?l#L››Qs?…7·"Uм?l#L››Qg4FGL J1631.0-5302?ëª[W†RÀ	ú D®…ºÀ9›)"N>À;3+­,ô@
fÑ@OÙâ_I?ÉÏìçÊT"?Ç¡¼}Ê0:?ÿÃ¥¦î?þ,iˆïú?ï—c"$ӿ犻°DÖÊ¿æÄS­úпëoÖ½—'¿É¥ì8Lø¿ïÿxáh:QAGNbcuPMN J1631-5256?í¿9X…üq?²ÚÕ¦²ž?²5;Ðw?²ÚÕ¦²ž?íÉóõ7¥‡?À"çüäM?±°`VBÓÅ?À"çüäL?è™qûŒ&Í?²:Š%#är?͚8ÏdÌ?²:Š%#äs?ê–ôÒxX?³<ê%	•j?Ť,·Â¡?³<ê%	•i4FGL J1631.2+4926?ÝÓû)#'@E`GýœÀ;$›À»GÀ<¨a¦
Ec@O+†®@ëU¹oø¶?ÉÀˆÊ>}?¿à¤ø?òéÆؗ?øµñ–°±
?ï*u¿á+3Šq¿í'ÿò> ¿Ç×ϊAaõ¿ïî¡UЗ¿ê;+ðHÒØAGNfsrqTXS 1629+495?ï¥Ðþ²^?=H¶¦4?†‹øSh©?=H¶¦4?íÃüÄ÷ò?º)[T±?±àØG~?º)[T¯?ï3o¸åп?'{%g3ÆÈ?™'ãEèP?'{%g3ÆÊ?ë[]
RÂ?®ßuî4?'‹Ö´÷©?®ßuî44FGL J1631.2+1046?ÌU°¬!@Aü¸{Üð0À9ÌöÕ´ÒÛÀ<&ç­"ãZ@0&îV_]@->" 
Q?¹ñ:j_k?Á!Í°!›@^¡£SW@ÿ³ÿÌT?ïýZž²O¿à‰xïÕæQ¿çYߥ¥^¿â-¸j?8û¿í;‰]â3f¿Õ:Ûs-ÊAGNbcu3FGL J1630.8+1047MG1 J163119+1051?ïËR&ºµ?fã"?zVì¢ô%í?fã"?ïõT)áÍ?hØ´n¸"Å?UÃW¬<dÆ?hØ´n¸"Ã?ïo—¥4²k?‰ŽD?<v1?'
Yi²·?‰ŽD?<v/?ïNj˜—?~[FQ"_
?–2¬ÿ.
.?~[FQ"_4FGL J1632.2+0854?êó·^@AuT\x¦ÛÀ:7,ÅÇÀ<Eq±ôr@qjKÎ4¬@*"³‰.è?ºæPA
$?"'CoÏ?Ûå'`À48@
X!þ­o¿¾63Úg?¿è(ÝnÛî¿ä+3Šq¿ãg&f¿R¿éïm«Õ€?Œò"‡$çAGNbcuNVSS J163211+085608?ïó"m[?QŽ02³æ?X÷ñ%ÏJ?QŽ02³æŸ?ïþY›R²†?D#ç0^v$?*fJÔ׶î?D#ç0^v.?ïÌuÄPo¼?çúúáà?yÅ×È!è?çúúáâ?ïø=A°Ø??{;;yT?O»
ù<¡Â??{;;y4FGL J1632.4+5800?ï!´s@Dzl <K
À;Ҙö«;À=µ?è@ Æ*ÚI7,?ýPaâs'??ÑEZ}$
?±‰Ä6Š?âi¿aTXÈ@Hñ0.q¿æ7­wa¿î-Ƭø/¿ÃÚÓÍ$á¿ã@9¿Ü0Ý£3Ì5?"gâèB3AGNbcu1RXS J163213.2+580109?ïÿ3X¥'×?Lõ1]e?"ëMÅ?Lõ1]"?ïþWaa@Ž?DÛuéò?*‰éë÷ù?DÛuéÙ?ïëúíÍUM?vœµ5+1?d2ª²—?vœµ5+/?ïý$øÓñi?*r9½©K%?6Ø9`t¸G?*r9½©KI4FGL J1632.8-1048?㣃–gV@8Mqâ›k+À9Ï0âöÚ½À;ÆQ°Ì¼@),P•ï–@Z䢬gÒ?ÂʌU¹E?Àɽ£ºò?úTâ_ܪ@"šÞ=7™?ﯷjdù¿âº¾ý×0Ô¿è';2ô¿å¶<'gN¿îŸ™Þb÷F¿ïö±½|ͱAGNbcuTXS 1630-107?ïð6ì¥?a'êJ[–×?^ý'&µØé?a'êJ[–Õ?ïýo"Ų?L©îØwB:?4ƒÙÒoX^?L©îØwB(?ï8F6ȲD?'(Ê,¢?˜÷9&鷆?'(Ê,¢?ïýìdQ¾Þ? Ÿƒ¾Ž˜?0œÝr	ß? Ÿƒ¾Žä4FGL J1633.8+0701¿æÆKן4[@@Ú4üaÀ:>*ՖŸêÀ<QÑææT@<~"ÛH@½'Óh'?¿XÊ`OºÂ?¶ÿ¬ž6?÷vÙ˸З@	'øŒn7ì?ïŽ!ÛòÚ¿º½¿~/°È¿à©(ü¯i¿ánÄÙ¹D¿ä÷K[H%3¿êÇ/~ó¦AGNbcuNVSS J163350+065705?ïúø¨[ÐR?=›
ô??D^¾¼Ÿ?=›
ôa?ïüÐþ½•È?QãÙbôSå?9x
Q¼?QãÙbôSÙ?ïåÃ|©ho?tRQ")n?j<ƒV—'?tRQ")i?ïÉÜêzN—?b↑œL?{ŠÂØ´š?b↑œN4FGL J1634.9+1222¿ì…ûþâæ@Aé4?¢­?À:øÓêÎ?"À<dInÞÛ@ #4ÔžÓ@(ã«5£?»­¢e6¿¸>Ú 
ëÀ@‰2"Ѽ?ûž"Ør}?ïûlb&¿è¢µ6®÷¿ã #Uož¿îû9Ç¡ê¡?âòc"úÎh¿ðAGNbcuNVSS J163502+122142?ïþ‹môø?@dO%Iô?'I °xO?@dO%Iô?ïâÊŠêä?ÄÓaHÚY?m5úuZ?ÄÓaHÚX?ïRá§gf2?QÒ
(¥!?•£Ë9Î?QÒ
(¥ ?ïj4H
º?LX¡¾_Ý?'¹vþ^èÒ?LX¡¾_Þ4FGL J1635.2+3808¿ÅbÃLÔWÔ@E*â:¸cÀ6K¯*ûVÀ;	ÇÿÞr@Ÿæè%@£$\֚¬?"}Y"M?ÀMfûŒ¨Å@4 uĨ;@!›fçÀ™¿ÉTå ig¿át·AË&"¿ælÐxR÷õ¿çP¼ R;¿ë·
è`Ý¿ïÿõïùAGNFSRQ3FGL J1635.2+38094C +38.41?ïÁ?‹ãþ¬?} %Ü{m?`:©¸?} %Ü{l?äkZå¡?Ûjn<Ð?Öý)KÀ4¾?Ûjn<Ï?îSîC¦j?¢)À\ì??¯úÁřR?¢)À\ì@?"JŽd"î?™Ùû3÷êÔ?ïe«ŒÛb?™Ùû3÷êÔ4FGL J1635.6+3500?î–ˆáš@Dü¼œÓà½À<¦-%ÒøÀ='ž>Dn@Õ³¦53@÷C˜Ü?Údò=I·"?ï*~ŸBP@.ðþÛ<Ò@Çy–™ßæ¿ïqÞ?ïýnŠø'¿Á‹½ãÐÊ]¿ãàâΖÑh¿ïÿx@XŠ±?å(@[9âzAGNbcuMG2 J163505+3458?êÅÝô Áø?ƹ¿Â"£?Äèˆ/|ø ?ƹ¿Â"£?铀íϘ?Íï¿óÝØ?ɱüKÐÁ¥?Íï¿óÝÙ?ç'fašè?¸_@«ž?ÑðÝ3<Ê0?¸_@«Ÿ?ãu
[N*Ì?½›µŠ¯¡?ÙëIcªh?½›µŠ¯¡4FGL J1635.6+3628¿åÅRóÔaE@E"î9.À: á$r¦À<	t"&"@wæ£ãt"@ë&T' ?º0@åxjJ¿ªµèž~I¡?ënþ…¬|Ë@ªÖÍvì¿æM˜9GIk¿åcÉ2äXÛ¿æÞ£ßm¹A¿äõ'ÊIdοïÿö$´ë/?îï'Á8AGNfsrqMG3 J163554+3629?ïþo¯'j?/Dö°D'^?)Ù_¶f?/Dö°D'Œ?ïý®ú
D?Jwˆ'	ö?2ˆ/¯eØÞ?Jwˆ'
?ï±³x[ï?'Vêᵖí?ƒ"!é;Ð?'Vêᵖç?ïÿÎgÃ>ôî8éUV†>øöÌsXš>ôî8éUT¼4FGL J1636.3+7128¿ï|ÛÆa@BbA=·ñÀ:ê‰Ê½fÀ<šlvJà@G`Ö@r$'–GÖ?»ÆUˎ‰¿¾4b2O2˜?ýûk{y"@•àZôi?ïøf–=ï¿ç_·ö{ó¿ëô(üxŒ¿á;Þ}yR|¿á@W¥ÙC¿ïÿèã«6AGNbcu7C 1636+7134?ïîÀ-\—V?jÔ¦hºf?a?Ò£h¨˜?jÔ¦hº`?ï°1Z§è£?›d]a֛?ƒó©V×:?›d]a֛?îü€q©å}?"æƒB	Ì? 7øåa¨,?"æƒB	Ì?ï[«¸]ê?‰NNUS-?"ŠˆôB¾?‰NNUS-4FGL J1636.5-0454?Ô_
Ê$@:óúã`	À;"ˆ\ÙöÀ<XùD$?@!ñ¨Ôõæ?ü—ù1~'?Ó3®BÈý_?¨$ j»'?Ñ» |ø#@G6·!>ê¿å›¥"
ñÛ¿íàœ…˜?ÅYGŸœ¾¿æhãï(Ah¿ÑßÇ[Ýá¿Ï…òGۋ×AGNbcuNVSS J163631-045506?ïþ0–êÄ?.dõ_o?/œö'Sº¶?.dõ_×?ïþ#›¾x?EÐÆ-Xž?-ÆD~ô•?EÐÆ-X'?ïßۘ‹ª¶?qÆt^æ4å?p3º*¤"?qÆt^æ4é?ïîýºµ•ü?Uòzwx™ö?aEJjÝ?Uòzwx™ù4FGL J1636.7+2627¿Ðg™ö|Ði@DŒÁDŽÀ:Q÷·\"@À<§".Î@âPÑQl@ÉuDO»)?¾i®oišM?¹
·ß»øû?ûŠYUëÒ?ùgÐáÚP?ïþ˜â9›'¿Þ†#3‹É¿ã<b0÷š¿âgpÛs¿á³´,ÂÖª¿ïëÿÝÆDHAGNbll3FGL J1636.7+2624NVSS J163651+262657?ïäøȏ
™?lI "6?k7põfH?lI "5þ?îP(=	Éx?±"1«Ÿ¡»?ªý|/ch†?±"1«Ÿ¡»?ï"üÅ¡Ù(?ˆÊË`W&?ŽÀΗ‰¶,?ˆÊË`W&‰?肘,¡^?«—Ë;ª—?ÍõŸM{âŠ?«—Ë;ª—4FGL J1636.9-4103¿ìBlÚi€Ö@€ÙÃUTÆÀ9zþ‡YûõÀ;)'o(¬Ç@{1ÊÓMo@Æۙj?ÈWÔþ©c?Ètè_Op×@òyÝ;¯Ù@ÊsѳçN?ïÿÖyô¸¤¿Ã¸«Ãã¿èùD$>û¿ä?˂þž¿ç|éàƒãпïúšï°AGNbcuPMN J1636-4101?ëiñËl³ó?µ`sPŠõ?ÂX8ÒM02?µ`sPŠõ?â÷CŽ,M|?Ó~VQ®´?Úxã§e	?Ó~VQ®´?çx
»d»?¹aƧAæq?Ñõê‰6‹?¹aƧAæq?楃BsU?µÃ0M"·?ÓØ´ù{W?µÃ0M"·4FGL J1637.1+1316?ÇóàÎsEC@AÚ!xöŒÀ:úmPes!À<sÝo²?ƒ@SØæ
¶@u ÝD?Î4rÎSµŠ?¸"éclâ?îD½¿h¶"?üÛr<2‹C?ï³hëÒ¿áúóPÅr¿ä&Iàô¡þ¿Ö놡D]Ó¿êàˆ!ö¿ïÿý`éNäAGNbll3FGL J1637.1+13141RXS J163717.1+131418?ïù6¢n™?O	3e²ö?K%w–E˜¢?O	3e²ï?–
qœ?˜ûÌt?[?ˆZ|£™M?˜ûÌt?\?OyÔ¥?‡Œ¯ëÍ°˜?‰˜l!ŠÖd?‡Œ¯ëÍ°?íüoRïÓ»?'|NÀB?°…hb?'|NÀB4FGL J1637.2+4327?å¡+§›Ñ¹@E
ÆûÒsÖÀ;ÙPVY¨éÀ=y_gn¤@!'ïCš3?õA³(¶Ø?â`€É>"?Þ´Ù% £y?ý	µU·Âz?ìsö™Ïտߝf'Ú?ì8ŸÎz¿Ø"€ð«N?µÊ£QÔ3¿ÝÜ°Úþ¾·¿å95Á-sAGNbll1RXS J163711.1+432548?, 8;?¬¦°È½÷ø?‹Qt÷ññ;?¬¦°È½÷ø?îªù›¥ùC?¶°
Ç?¥PfE kâ?¶°
Ç?ïN;'?Ì¦o7Æ?–?ü½Øç?Ì¦o7Ê?ê¹'e†?°Ù{îBt?Ç¡¶iç?°Ù{îBs4FGL J1637.6+4548¿æ7£Eºp@Dý\B 6À;©%ʔä(À<ùZ'ó+@!¯…>BÜ?þ¡YKË°m?Ëz©u¯°?OöìˆZÖ?«¾œ!M€@~3ˆ˜•c¿ïÿT•Ð·?ïÉL¯Ûû>¿ãÆ'+½óì¿éC•ìeïH?ÔÉJ àuK¿ÛÈ…3[!AGNbllB3 1635+458?ïýTþ-¸?7™"ÔÓ¬ô?5Xþ'7ý?7™"ÔÓ¬¾?ïþ W/E?GÀdšÅÞ¹?/ýúƃ?GÀdšÅÞ×?ï¹ÐÈ-¥?´u½›õ?‹Íô¹w?´u½›ô?ïüÐIÁk?3AáçH ?9}·Aô?3AáçHŽ4FGL J1637.7+4717¿Ø<Ý\E.@@DðÀƒn˜À8Þ©°â‹À<Aæh2ï@LtQ‹è@,Âþí±I?¢RFýHY?¬&|w"@¦#×þ@¹Ûÿð'¿ÂGpÂ_ág¿äv‹AèÜ¿æ8o'Á¿åM
švX¿è!£=Ý0G¿ëZA"õÆAGNfsrq3FGL J1637.7+47154C +47.44?ïûçiLÍ[?=Ž-E
?(?@bZÌʕ'?=Ž-E
??ïùÅr*¾?i#yLÃsÃ?Hê7UÁ|?i#yLÃsÅ?ïÕí©µµ?sq°HéUæ?u	+%%x?sq°HéUê?ïÿÄÔO{>õ"AYÄ	>ýøØB¤>õ"AYÁ™4FGL J1637.7+7326?æ;èÓr`@Aœa|ÚQÀ;»`iÍ#4À= á÷×=@ ÐåZ7Y?ú̓ÜÁ6—?Ñ&Ÿ|¶¨?ÌßI¼ŒÂ?ùñÅû!sî@g°'£#¿î@5¯å5y?ïÛù%k¼¿á2:DŸlA?Ää^ú6gp¿é–Š ØR<?—çCp˜AGNbll3FGL J1637.8+7325RX J1637.9+7326?ïûÎIxû?BæSßÂ*ú?@ÆÚÉ ?BæSßÂ+?ïý0½V?XtÿCžpš?7îzOJÒ?XtÿCžp¢?ïV*»##h?ÿޕžc[?•:¨››"'?ÿޕžc[?ïû¯E~.z?8¶ÓFH'œ?ABêFO?8¶ÓFH'­4FGL J1637.8-3449?Øh…ퟛ{@ L׌CoÁÀ8ì=áâßÀ;²ïQ/@ h½1øv?ý"
¹&&Û?°?lÒf>Î?³a(c÷KQ@¹üȽ@ŠT©$¦þ?ïìæè×ÅN¿ã2´ˆ2i	¿ÜÀþè(¿ÕN]Ƅ´/¿à¾há?öe¿à2ö—¡qÕAGNbll3FGL J1637.6-3449NVSS J163750-344915?ïûËcî¼t?7}Ü
2r?@ÒpE.Õ?7}Ü
2©?ﯝ5qsù?œ‡£Âj?"²££Á?œ‡£Âj?ïÍ:7Ì¿?ƒxq+ÍÒ?ybòd ?ƒxq+ÍÑ?îŽ>Vã‡7?"<7õ
?§'ÇŒž?"<7õ4FGL J1638.0+0042¿Ö¹2Óáä@=¦ë¢zé«À;-¸éÀ<‰¿1×@"(Z)ÂC?úTœ×%?Ìvì…ú«W?©T"¢Í±
?àÖJ>ès@]/Ûæ¿é««Ÿ«y?ïÿY²"ý[¿èöÝÂhp?¯p
BèÌ¡¿ä
Cë[r¿Æ¨Ã
†AGNbcuNVSS J163809+004223?ïþá.ºé?"!þšüi%?'íQx4?"!þšüi?ïûš¦_Ü»?[{é×(‡ï?A•f€<?[{é×(‡Ô?ïïgy®?_ÖÀfۍ?`˜÷†êP³?_ÖÀfێ?ïÎÞÖÛËÖ?lËi§42:?x"'†?lËi§42?4FGL J1638.1+5721?Ñ;
՞ŠÑ@D/ŽèÀ9Í|ÉV À<†ŸJ³'y@;Y:Æ@Ü6r?±¦îýàQJ?³
è³³ ?übÏØðÇ~@°ŠÖ2Q6?ÑÓ-äê¥Ñ¿çßÂ=&Ñü¿æôV2ì¿ë
`¬B"¿ãæò}`}ï¿ïÿ7J³AGNfsrq3FGL J1637.9+5719OS 562?ïÿš"Ԁ?…n ¨]?»¥oêÇ?…n ©C?ïý¥Lb…å?EÏÖà†é]?2՜ëÐÔ ?EÏÖà†éh?ïہõ•?nˆ\T¥?r?~…u5+?nˆ\T—?ïú›ôr€?6M,›5?E"".5ÿË?6M,›(4FGL J1639.2+4129¿îhg£w3@D܁Ü
²pÀ:^þُRïÀ<HKv @õõ0Ä@ˆœä§´å?ÃDuû°?Ðìà=—æ@
ί%@8у?ïþ@bEÅ\¿Ý݅íjñ¿âÁ}
q؊¿é!¿îB¿ëK¿Ê߀ƒž¸AGNfsrq3FGL J1639.8+4125MG4 J163918+4127?ï¦ù	0?Håý"—?†Á½³øì?Håý"•?ïùíð¬›?hÅÅۜ
?HH?ÍM"?hÅÅۜ?éÔýmö\5?±
N
Â÷1?Ȭ
H&-?±
N
Â÷0?ïâ*òŸeÀ?X¨ïpH½?mÕ
`šA5?X¨ïpH·4FGL J1640.2+0629¿ÜüÍ ÀD@@*Ã") À:º$§5jÀ<f®ITè@!P5©/8Ó?ý}<9Aj?¿Ž9ø¹¿r2byíŽ?´; C¦7@ùùü/æÍ¿èÈEßÞ"?êBÀh Ó¿åù#7<­/¿Þº/(¸¿ÖoïœZ" ¿Ô1"\p™EAGNbcuNVSS J164011+062827?ï÷'«ßi×?JÖÐÛe'Ð?PܨA,R?JÖÐÛe'Õ?ïüÆÈú<?Rã?:´y­?9ɸ/ù?Rã?:´y£?ïï8¿§Q¶?eg4iìPs?`Ç@X®Jm?eg4iìPU?ïÒà
_ç€?fw`Bi3Á?vùP?Á?fw`Bi3Å4FGL J1640.3+6850?ï¶oªî2¢@BgNe¾ ºÀ:ÃfÓ'ºÀ<ō²Û‰ÿ@(j[i@PÒÆÒí?¹Ö°™†¿ %üCÕ9?åƒí€ ¡¶@š¥'Ÿz.?ï¦Eÿ¾'¡¿ãxK é'¿åMåр´¿á¬4Á
!¿ÜÈ+'¢"¿ÝmHmWpAGNbcuNVSS J164014+685231?ïþõ'CoÎ?(àض*`? ­‹É9ˆ?(àض*ä?ïþj"ô¾Á?BZc nYÌ?)W°´ò©?BZc nYì?ïùæÚ™?_u`šÏÎî?Hd—ƒù›?_u`šÏÏ?ïü8+wH?*)œê)p?>>¤Cõ¾¿?*)œê)4FGL J1640.4+3945?ë¾7fìK¢@D¶¸ºÇÀ8T¢eðõ¡À;r:?–îÄ@àðÎ^È@ ðÀÇÛÌ?§É·n–¶?®ùQ~ç€q@ÂÈ>Ȓ«@úÕOӿܤ–LÝÿ$¿æz8«B8Š¿åÜ7£Û<¿å3"6‹­H¿çþŒ}Qdw¿ï>ÎÝHEAGNFSRQ3FGL J1640.6+3945NRAO 512?ïøsÇ[1í?K®TvJb˜?N0â"8J¼?K®TvJb™?ïû+¼û²u?X¡"G?CQ61¥?X¡"R?ïgÄm9œ?žÏ@ÍçÂ?"GrXÌs?žÏ@ÍçÆ?ïþ‡ÛŠ? œÜ eiL?'Ž"N§s²? œÜ eiÅ4FGL J1640.9+1143¿ë÷/Bg8@AJýTTÀ:%ïpeéÀ<?gÀÙyƒ@;‰³¢x@?Tú-X(?·(xD4b]¿DË*ؓ ü@'drñ9¿é¦Ž¼-ÿØWv¿$·¿èt­Q'Ñ¿ä0œJNì¿çâC5à?ª	CÜ´Ý~AGNbll3FGL J1640.9+1142TXS 1638+118?ï­øÍ`&f?"^»3kã?"Ì§öfi?"^»3kã?ïûhtêW?]n@Å?#Ì?B_Þ,V¦š?]n@Å?#Ñ?ï	E䫪Î?'<
eÅ?ž×CjŠ¦u?'<
eÅ?ïÆ(»­á?lm»'ŽÜ&?|÷k¢)ù?lm»'ŽÜ'4FGL J1641.9-0621¿Æ¾Oj®)~@9íÇïzÀ9'-åìXƒÀ;©pÑ#s£@
+¢F¨@68ù€Š?·EH´yĽ?ºþð¶`ú—@Wš»ØˆÃ@
ÉÂK"}ü?ïKøQÆ¿Õ}Þ€iG¿âÄßÎ1PÛ¿á߆®Š©¿êb…Ñe¸Á¿ïÿÿ" 5•AGNbll3FGL J1641.8-0619TXS 1639-062?ïÍtïh¤?x¸r°wR>?yEˆKû­Z?x¸r°wR<?ïö†×n x?fëˆäCƒ;?RòQ"¿6?fëˆäCƒA?îrm/3?›$Á\ºŠ?¨Ù-Ïß?›$Á\º‹?ï<£0¯?€ˆÛƒbôó?˜kŸ_¹ê?€ˆÛƒbôò4FGL J1642.3-8108¿ïÿÿôw
3À6+¢±pPÀ:ŸØvN:öÀ<$iϘ@«FjGœw@âWãì¤?À<'ùn@z¿¬\[p¿?ëXm_)]@ã%Íïâ|?ᄅSK¯¿ãI€2Wk¿íeK´3xÓ¿ä¡ãÀ¿ ;ƒ'¬¿ç·fÔJoAGNbllPKS 1633-810?ïóG7µ¡?Z ""Þ?YÓq"¿+?Z ""Þ?ïýã]L{?U=ZeV,E?0åŸd0B?U=ZeV,P?ï—ÁF/É?ƒø!‹é?Š®t;Î?ƒø!‹é?ïôϼM»?K
…Êâõ?V`‡ùd‰Õ?K
…Êâå4FGL J1642.4+2211¿ï˜xä@BÝE¶ÃvÀ;rŸ'*_OÀ<£fô*ߨ@!"…]ÓE@°"—©Õ?ÏWŠ€wË?¬"OÓ|ê6?äØ°?ù?G@ž×ÈSkb¿îj.Ýc?ïü_#¦ù¿ëk><{±Q¿Ìm«ÿøž7¿á#ʪ³Q¿Ò^³ŸTC¤AGNbll1RXS J164220.4+221132?ïúPÝ­ˆí?Jó	"`û?F¼‰IÜLÏ?Jó	"`û?ïú6€sém?`—1n!l?G%þ0ZK…?`—1n!o?ïá%­§?mƒê‰ˆD[?nÚ=RáY?mƒê‰ˆD[?ïþÚG/F?q'y[%U?~ 'Üh]¸?q'y[%U4FGL J1642.9+3948?éا2vm÷@Dz'öè)JÀ89m;l½˜À;v†eà/@åëÛóÛ@dŸ¼ÉJ?£<!Þ?¥9w'.?ÿM€k_Ê@;ÿ>¹ú¿Ä©$&%Ä¿àXÔ!Õ½·¿æoP»v­¿åø˞#—	¿æ:%6ñ.¿àpë$¦¨vAGNFSRQ3FGL J1642.9+39503C 345?ïøÞp2²Ø?Jw½z!•?L†?54ž˜?Jw½z!…?ïûY"'?Z|Ÿ†¿Ù—?B››ýíÀÚ?Z|Ÿ†¿Ù•?ï_›DAo?'5, ¢æ'?"—wÞr?'5, ¢æ"?ïûI‡F?8¹-¿?BÙâ烉Ã?8¹-º4FGL J1643.0+3223¿í皈ôËÓ@DC,¥zxÀ:»£?4É5À<#e_Ö)@ð¢S&˜›@üÄÞÁÂ?¿ôPßÁq$¿¡¾ò!M¶?áÓÆÞ@•Æ5ƒðe?ïôŸhËÆ¿éŠÃ=O¿â…yA	Š˜¿Ý|þ®F¿í™z"¿ï÷Ê! áøAGNbllNVSS J164301+322104?ïĉ\;k?y,‹'ÎÌÙ?}ó;QâJ¨?y,‹'ÎÌÛ?ïíépí°?vu¯}¬`?b<RO?vu¯}¬c?ïcÏaQ?Žñ_Û´ï"?"Ÿ¼æÕ¾?Žñ_Û´ï?ïEPTN i?"–æ4´‰?—Uõv+ó?"–æ4´‡4FGL J1643.0-7714?ï
‰e(ÈÀ3æ‰enï¢À:Ϻ×5À<*•Þ#6f@ì¾ÝöÀ¼@$@Q(ç?ìÛÀ°Š¿¥IÞ}â?äxdFÑv?ÿIkjÏ?Ý퍁Þ<¿Õgˆ$|61¿ìÍÛ?¬=`¿Ü³Š;WÄã¿Ð¿'zç&ë¿ïÿüoQÇsAGNbllPKS 1636-77?ïî†"n'E?b²5c¼?ayݑn¼b?b²5c¼?ïà$¥hÉp?‰«y0;?oÛZ—6Q?‰«y0<?ï_>ž¦È?‹!=;cì@?"˜,+&õ?‹!=;cìB?ïÌ N³ó?g+HC€Ü?y¯Ø¦y_?g+HC€Þ4FGL J1643.5-0646¿ÔTÈÔºÿƒ@8xoš™tÀ:/<"댫À;ç–{(@ 1"­ú#È@
*áU?À­ŽÙw*.?*äâð?ÃÂ
V)ØA@ÊÑGZÝq¿»z£à…¸¿êßJþ«í¿å.iՆ¯²¿ßµ×<è=¿ä?z™¤¿ØÊ=fAGNbll3FGL J1643.6-0642NVSS J164328-064619?ïüªP	Ø?6Ê5iãø?:­ϱHH?6Ê5iãã?ïþýmþ7Ï??ÿ/ÒâU? ) ƒÞ??ÿ/Òâd?ïã"Ò¥&Þ?v‡ß"®?ll-ZÙ!ü?v‡ß"¯?ïü½&M?,D"S76?:Ë÷ý•ü?,D"S7>4FGL J1643.7+3317¿‰¼BW¿Hâ@DÔk&¿‡À;œÑ¹ôƒÀ<æݝÕh}@"Yp)]Ç[?ó1°|4.?ݜöZ婽?ïþY!Yl@ÒÞ^ň@%4ºÇ¼˜?ïý*BsÂð¿ï›iGÂ6q?à´®ÈÕÇG?ᇆqž©¿»f͔ré¿å×táSlAGNbcuRX J1643.5+3316?ïÚ
FüL?wÄþîE·ï?rúó܁Ú3?wÄþîE·ó?ï䤼¬…?ˆ§QØHdÔ?kù[CS{<?ˆ§QØHdÒ?ï
ÁžFh<?"™-¥(j?ž§Ì72ø'?"™-¥(g?îlhþÛ$?¢Éagü†Ê?©9pOM·?¢Éagü†Ê4FGL J1644.2+4546¿ãÒ}ì`"M@DkŠC»À;hEÏ)èÀ<ð1Cnê™@ ºÞ؁â?ýÒ¥Ú¼j?Ȃõ}Åþ|?–g—á*?Ñiè;")@aÒ­âQ?ïï=Û,áà¿ãÃނ׶¿×ñʳ!¿âo‰û–忽àÿ´«˜Ë¿è-Ë_\ªAGNbllB3 1642+458?ïü™5ÜÒ-?7M¹âã.¨?;6Qn£Š?7M¹âã.Á?ïü÷ØpÔ?XúDìѪþ?8A<y_Ñ3?XúDìѪÿ?ïç®ÆmÌè?qþ…\ÛÕ?hQ9'3/?qþ…\ÛÝ?ïJã?P2<v½i?aÿJ@µ­?P2<v½f4FGL J1644.5-4602c?ï…ðæ׿Éýw¤ý%À8…‹W"<À9ï–
óފ@"#ÆX¿_@Ãûå¿?Êu´¸,?ڄ]<œ›@<Ÿ¡ñVð?øtÊÒ̖¿ïûŸH/Cº?ïåRj0'¿â8Y­ñ?s¿é˜´—Ká¿ïÿý±q&´?ïÿŒýÿʦAGNbcu2MASS J16444975-4559026!?àŽš 9?Ù¸Ôpí‹?ßÖãþË¿?Ù¸ÔpíŒ?£	+fX®ª?º‹Ûÿ»Vç?îÏmIšu?º‹Ûÿ»Vç?²9(ó+çœ?¢L;ÒK?í¸Úᚃ?¢L;ÒK?o;¤ERæ,?fO Nr?ïàÄ[º­?fO Nr4FGL J1644.8-2154c?îøí²P±@.}¶™"¡À9ώ—"À;VqÐý³õ@ô¸ßÚñ~@§¸
è´?Ä~eá†BO?©©žŸgäÁ?èyØÔB@ÐUjÀ".?ïþ'ýž%ð¿ÛåB{¥"¿ä'Ö÷ÈùÙ¿æ Üš*¹¿ßr&s!á¿ë†hšMAGNbcu2FGL J1645.7-2148cPMN J1644-21560?ïµ =-Ÿ?`\†ƒTŒ?'·ù0´˜?`\†ƒT?!Ž¹-?žæ¡ž°´?ˆ÷œQ´Ñ?žæ¡ž°²?í_§½²½'?£'èÒQ,@?µÂjn?£'èÒQ,A?îósÐÇÌ}?ˆø8zj¾? ÈÂóƒ8G?ˆø8zj¾4FGL J1644.9+2620¿ä©Mûó=@C.}=BÀ:T¨ÎÀÃÀ<NŒÂÂ#@1:¥mbY@ѓpŠ¬—?»ÍÆFö´?´"»;)÷ ?ôØ/ž‹q@
öäñ0Ú=¿Ûdï"¸Ó¿æ}U–4Š¿ê"n§}‡ë¿èç2^wÿð?ïÿٟC&ÆAGNNLSY13FGL J1644.4+2632MG2 J164443+2618?ïþ½cöì{?&¿‰h)<?$)À'8?Ý?&¿‰h(º?ïû'þ|V?ió<}÷K?Aô£Š?ió<}÷Q?ïÜ6ÅqQR?qqĨÿr¸?qäGWVÚ?qqĨÿr¼?ïøÀ£ó²?Bkúŧïý?Lýùp11D?Bkúŧð4FGL J1645.6+6329?ïhþ
Åõ@Bü½º
RiÀ9á07Ö0#À<hœo6ï€@T—Äw#@
‰ÎÒa?´¯[ø¤A?ÆãÛÅ~@<œÆtÃ÷@T)`vP¿Ó‹¾úýÚ¿àö4êK¿æ,%!øxL¿ë´×Á¯b¿çj¯Áy1š¿ïà18‡0AGNfsrq3FGL J1645.9+6336TXS 1645+635?ïúañæ¢l?Iƒ4ÃOU?Fx8evN?Iƒ4ÃOi?ïùTA9N?bJŒ¼n§s?J®ûžÄþ?bJŒ¼n§v?î±d៓Ë?–û˅åxO?¤é±æÃX?–û˅åxR?ïô…ÎOvÛ?EþŒZQõ?VôcaH‹?EþŒZQò4FGL J1646.0-0942¿à÷´À´q@6Lp¸Ï¿ÆÀ:¬~T–ZÀ<®Ò@!2ëÇ@¦¶~¡Ç?ÀÝYâÊe¿©—ÿ™jË?êᡥו~@":îéW¿´Îž31ZÁ¿ìÔ)þ+>¿Ïؓ)'ög¿çÀXëS '¿©à¡•ø‹¿åý
a½_GAGNbcu1RXS J164602.3-094113?ïØv>ñ?rU¼Ê¾Í?sÄøà‡rm?rU¼Ê¾Í?ïü|¸kS?] ì0'|?<<¥p9?] ì0'"?ïRžÎè?ŠÎIW?‹ø«XLF=?ŠÎIW ?ïЖ‰w!ý?i۟4:™?w´»Do^?i۟4:"4FGL J1646.6+7422?ïçƒ×@G@A$'žùTëÀ;^#QA;À<ñÄ>ˆÑË@ï·=ïNØ@=â@ÒX'?Îð颜Ž?Èùª¦\J¯?÷ôt{Òß6@˜5ÁWú?ï°û€>~Á?Ù=B äfœ¿åoïaLK2¿âhˆ•â¿ä²¥¤i×4¿áþ·á-VûAGNbcu7C 1647+7424?ïö†3Ix~?Uhtêt#?Ró™mü?Uhtêt?ïü"tt?T…CÙX(?;ßô_gw?T…CÙX?ï‡Öה«î?ˆÿ]qä]?Ž
JÕx?ˆÿ]qä]?ïÑÉiÜý?cEÎ	4ýÀ?wx›KØ?cEÎ	4ý·4FGL J1646.7-1330?ޕpoÑXó@3õZž²OÀ:ΐTvyÚÀ<)VlGQ@"m@JGø?þ¼I	^N?ƂcÇûÁ¿—ú¹š?Ð$ñüÝ
Ý@/¦(s<?ïüÇ0«™v¿éó5ò*T¿ëOŸ_¬8?'3CaK¿âFîœ*m'?¯¾
þV˜ÏAGNbcu3FGL J1646.9-1332TXS 1644-133?ïþd–'4Z?1ˆMV,J?)¶—ܺeT?1ˆMV,U?ïüö™¥¼Ð?U¥ªå-º£?8K2Òx1?U¥ªå-º©?ïâ¡òـÒ?t¹9_GÚ?m^
&-ì?t¹9_G×?ïõ™ìÈ?G_oF¬êå?TÌ'ñònÎ?G_oF¬êØ4FGL J1647.0+6040¿ê‰+"þƒ@CAÚßµÝÀ;s €©ÌÀ<Äæ©å@àfgh@±ì¹ÒE?ËD௭­¿vÓÿŠÓòË?¬1¦|g?æ@5=†Å¿ïÜD¿L±‰?ïRuÚ¿èsûÿwD¿Û+κã–=¿äèÏÍ2MZ¿ç‡Jw—AGNbcuNVSS J164641+603930?ïõy?c!?Zàµf‹t'?Tý
9¿¼?Zàµf‹tœ?ïþ(ï›3ó?Døî'gXk?-qLÀϧ?Døî'gXr?ï\ú"¿t?†ÔýZ?ˆ¨ÁZÐ#?†ÔýZ ?ï÷©Üx™?AýÉÃää?P¬GÏΪ?AýÉÃäæ4FGL J1647.1+6149¿åG EeøÓ@Cvÿ:Þ"À;AºrW5qÀ<éegÊ@:¹•?úƒŠéÓmÑ?Ôª;þ2öL?ÔzJ´Y8€?ûϨ´¿Í@G¢ŠY
?ïý#I±$¿íÙÁY|¿Ëì쥿ÖÍ.œ=¹¿ëuäޑpU¿Ò|¾aÏþ°AGNbllRX J1647.3+6153?ï÷úÿ J¸?\µ‰+¸ª"?P
¿jŽ²?\µ‰+¸ª ?ïü/d"´'?Vƒxe³U?>"Þê[ä«?Vƒxe³M?îé"ef4A?"'Ét͑\?¡mÙ©œ»ñ?"'Ét͑\?ïÊ'콛?de›"ýrn?zì{‰¡2 ?de›"ýrm4FGL J1647.4-6438¿ÁÅ,‹WwWÀ(íêî ¬À9€éNã'âÀ<fåè&Å@4$ÕwkF@
¿@óW?±.q,"?§(¹vÙ¦?õA¼bò@ˆWƒŸ‡D?ïñ?Ù}¿à"P&‰Å¿å"ÈL4‹ù¿ãJ=Á+®Ú¿éˆŽ^Òô.¿§™(¬AGNbcu3FGL J1647.1-6438PMN J1647-6437?ïóWp´fA?Uþ3ҝ?YQ—3|?Uþ3ҝ?ïûêµÚd'?a'‹"©o`?@U(–m¹½?a'‹"©o\?ïÇÍOÆ?}µÌofO¸?|XqñÖ?}µÌofO°?ïç,FR­þ?T꼒¦¨&?hÓ¹­R?T꼒¦¨"4FGL J1647.5+2911?îdÓïàs$@C='Ýãu†À:É@š$À<gzbœ­@Ë["l@{k{y"?½†ý )Uº¿¥2!BùWx?è:±âe»F@öü¢R{¿ÔÖß?–¿é£(Ž"ƒ¿àSþO%Ø¿çOÞk…µ¿Ò34	òÈ	¿â^"3N&AGNbllB2 1645+29?ïø÷®s?J©Ÿ´l>?O!F3˜Õ?J©Ÿ´l4?ïþ½íz²?G¸s#TÃ?/!(TÓV?G¸s#Tº?ïß,xµˆ;?t‹à¢-?piÃ¥;â3?t‹à¢,ý?ïöôáMŊ?A‹µÎTFb?R=dtî?A‹µÎTF\4FGL J1647.5+4950?Ô^A{í B@D	õ­–¦ À8ú'ûnjÀ<GùsôÄc@Ô)«|ñ@î¸D‹Ñ?¢²o~hß?Ÿ}ÀzNŒ?ôQ.ül͉@3L´äx»¿¸þö?·Ðç¿âíæÝð
¿¿æñਠñ¿äìö}Ë1í¿ã¼¡Ü^:H¿äÚ;JXêAGNbll3FGL J1647.4+4950SBS 1646+499?ïýzý㟜?+æAib?4(ã?+æAib?ïüûŽLu?OÄ\E\Žº?8#œW'¬?OÄ\E\Ž¢?ïì6Çͱ˜?jì-+ß(ó?cÉ82Ni)?jì-+ß(ù?ïý8<'/?,"OJ[KF?7ž>îŠ?,"OJ[KP4FGL J1648.0+2221¿å8ñ¬'`Z@BD±ëÕÀ:!Øb,EÀ<MˆGa¾a@¾úWI'ñ@7~0‡‡?ÁžsˆØ›?Ë$ƒB@† Ä0F@b=Í@:?˨c`øh\¿ãR@>´q¿é†k>'aí¿ç<ÛR¡"¿ïÿô¬å¦¸?ïÌ®.|NAGNbcuMG2 J164800+2224?ïƳR«?€ÆÈ-–Ê?|¦tóVªæ?€ÆÈ-–Ì?ïøivŚ?e‹þL"±?NZ$é—ÀÍ?e‹þL"«?îV<–>*'?œØ(O#?ªœ6œ]‹?œØ(O#?ïÍS¨z½§?kù"bå´ ?yV+¡,Õ?kù"bå´"4FGL J1648.2+4232¿Ú`áЎôg@DË)^žÀ9¸xq*å‡À<wÜygË@öO+â1
@0‹¹F?±àÀõ~å?´
šGiv?ý œ˜Q›@ýuOÐ?ïÿÿ>¹ú¿àW¤ª²¿æg9ª€¿å9‡`1&¿è¾uñô¤'¿ïáãµFžJAGNbcu3FGL J1648.0+4230NVSS J164831+423322?ïýßS#és?*¹µ]¥?1fà´o=?*¹µ]¥(?ïü;Žæíµ?T9&É6‡ô?>#ˆÈ'N‡?T9&É6‡î?ïË$=i4?uV{>Çwþ?zmáK{æ'?uV{>Çwý?ïýŠ'ÓÚk?#Ø¡CžþŽ?3«qa,¤'?#Ø¡Cžþe4FGL J1649.4+5235?²ø,å[î@Cĵ¢
ÜbÀ9*ÃÁ‹P+À<<ôE·š6@+Xäʑ@J¾A?¦?·>ßÓ?ª|·õ@EøÒåÂ@à?pXX¿Ü
²ûjo¿ßŸÀdµ¿âra ä½¿ÝN	îû̿䆃—¿¥¿åõ'ž}¯AGNbll3FGL J1649.4+523887GB 164812.2+524023?ïþ"´ ¿?"x-	aðb?&Ͻô3?"x-	að?ïü«ÿí·?Q¶°ýÝJ!?:§Ð'FÜ?Q¶°ýÝJ?ïñQ·Š?`Í×Á­?]\ì]?`Í×Á­?ïý@P\_?#!T^ŽX?3ý}>?#!T^ŽXA4FGL J1649.6+0411¿ïõêؘv@<åý2Æ&À:!$^"ÖÀ<	"&¸Ñ@J°7•Ãv@ürâu«~?ü}õ#X?ÆžÙtzü?þf"¿?E@Ý\"è¿ïÿÿ)@k*?ïÿúÁҝǿé¥Ñ¶@™M¿âO¬{­¿ïÿþó…õ?ïó˧nnAGNbcu3FGL J1650.0+0356PKS 1646+042?ïë'q'
o?'Kþa9ˆ(?dnŽmò=?'Kþa9ˆ)?ïûVßcHÃ?jà%DÍl?B¤'rÜù/?jà%DÍh?ìð´)5õ	?¦Ža80¬?¸z^¶PWÂ?¦Ža80­?ïöz[ð#?IÙN+œI…?SýH¹P?IÙN+œI4FGL J1650.3-5045¿ïÿÕfLËËÀÈ þÀ7ã',"³À;ýº@¾
/=…G@žÞ|øy#?¡ƒfÁþB?§bܙË@ô6%UúÞ@aŽQ?ïûûß	s¿äT^¦ÿ^¿åŒ|Dôü—¿ä÷'ê)Õ¿ä˜æ€Òù7¿å÷>àæ_EAGNbll3FGL J1650.2-5044PMN J1650-5044?ïù«sÞAm?I÷ü£B?IR0†úK,?I÷ü£H?ïýÆÏÌ<%?GwÕ-bP.?1ɁžÒÜ?GwÕ-bPC?ïnÁz~D?"§'˜›&?œ'а7T?"§'˜›'?ïüõ¦Gc?/2Rƒoxß?8RÏåÄÜ?/2Rƒoxì4FGL J1650.7+0831?·ùtR>ìz@>¥¸fä:¨À9²rùòŸÅÀ<<(¥:¸@Ñ
NG6@Øró<£?¼¸«­˜T?Ãy§¶½ÁÂ@°~ZxòZ@SaÅ¿ÀŽ|2iµ¿æï<™
' ¿äE`ýpه¿ê®HÌ]ç¿ì1  œWº¿ïÿÇ*Ì\eAGNfsrq3FGL J1650.8+0830MG1 J165034+0824?ïãJ¾8§?iÌcwŒ"?lµAÇXp.?iÌcwŒ{?ïû³t½M?T=$-ÙÔ?A3æ-
ш?T=$-ÙÔ?ïsõaŠÕ€?‹Qfnˆ[ñ?'SÎ¥P?‹Qfnˆ[ò?ï¿hwڛi?hâ>Ùz.î?€%â	Y%Ø?hâ>Ùz.ê4FGL J1650.9+0429¿ë€šMé@<À%á;ÛÀ;Zœ-ȐÀ<r¹¸óÑô@!a‰óß5Z?ü«+­,ôU?ЮúS?µJ;"ý¾?æ5™e—4@Ð}
œË¨?ïÝÅB"пîJn×N0¿Ö4œŸˆpý¿âBá[Ð
o¿"*å(Z´y¿ç"Ғßk5AGNbcu1RXS J165053.5+043009?ïþ×u55œ?!>9þœmá?"ˆ¬¬¦A±?!>9þœnO?ïýwìœu?O¼-wə?4G`›UD?O¼-wɊ?ïñƵOÓ?böâU£í>?]ør•`[?böâU£í)?ïålöµ¸
?]`¿É?å?j"	JG÷A?]`¿É?Ú4FGL J1651.6+7219¿êl¾vþ@AZ*o?RüÀ:u¤åýö;À<¨ÃФÉ@ €ç®z|H?ýùiÈñuú?µÕáswñÔ?sñ‡l?Á«Ü<Vr}@bô6H;ƒ?ïӟ县Õ@Q~Í»_¿â#îâvWJ¿á{ý§`+º¿Ø"ÿ^ow¿¼âÊ [PoAGNbll3FGL J1651.6+7219RX J1651.6+7218?ïü;2ñ¿?8oÊ)ßv?>&hrþD?8oÊ)ߥ?ïý~ÛO¸œ?NDõ%Ì®µ?4	%';Ø?NDõ%Ì®¨?ïë'–3oU?qwRím+?dØi̐«.?qwRím.?ïï±Æ\½ô?L}/îk0Ü?`N9£B
c?L}/îk0Ï4FGL J1652.7+4024¿X|Ïr!àY@Cb¯È°À:™":ÚÇaÀ<q.~˜ŒS@ Úàl'Ο?ýC$\֚¬?ÆuÌ4÷X'?´o"3,'?ñÙ«Ø`@ªÅ
¶'N?ê&둳ò
¿ãþÀZN¿Ï¥_ö_Ã4¿àXŠp0ꄿÜ®½î¸¿Þ˜âºtÛAGNbllRX J1652.7+4023?ïþ_ît%?"@çƒ&9?*(½µp?"@çƒ&&?ïý'¥sbu?KÜ¥€Ï…u?3rÔdìVê?KÜ¥€Ï…n?ïø|";äz?cC]MEçA?Nwn'?cC]MEçL?ïáÄóR¢?U¾drCªY?n;­ü^±?U¾drCªL4FGL J1653.8+3945?ç)O?¹@CmZ¯xþïÀ6Ę¹ŸÉ_À:½¿_ü¿Ú@7o¡Îqh?û‰¨U?†?‰i<¯ˆÄ4?"hKeP‰'@
gý?[`@0''àCÍ?Ú+Ú佄Z¿ÕÇ+£ù[¿Ü2Ÿæ¿g¿ÖPñ_(Y¿Þ"ÊÕ{Ç÷¿ÏU)¶³AGNBLL3FGL J1653.9+3945Mkn 501?ïô6ì
b?[c|IÈqŸ?W''å;ÃJ?[c|IÈq§?ïù×]Â?fÞËt´{?H£Š‹øö!?fÞËt´z?ï^*(Ï5?"5†µ¶?":¿æf?"5†µ¶?ïÿŸï>	Ñ?;1ðCOæ?0}‹U@?;1ðCPF4FGL J1654.0-3509¿ïêÿ"á@˜W€ðUhÀ9ª6CˆìÀ;'ã}zV@)Bnº@¾aÏþ°?½n'¥áP'?ªŸÀÊØM?ïºÿ?8$@Øד¥8ß?ïÿ®©Ì¿äÿà iA¿ãpWìPÓ¿à¬ÿ'¿çõò•´1Ë¿Ô©ãßVAGNbcuNVSS J165404-351301?ïËâl=?†l'áoù?zÉô}á¬?†l'áoù?ïÒÐR.÷ ?>‹ÓQÑ?v—Öè"p?>‹ÓQÑ?ïœ9º7^?"¿+€"%?žŒxȹ?"¿+€"$?îóFŒÊJM?‰BЋÕhI? Ë—3[[=?‰BЋÕhI4FGL J1656.0+2047¿îü œ7I<@A$äâmHÀ:!ãû½{ À<RNöÞ@-â´?¸'@ŋûKeY?Á'ï@À£?ɹÀ€Ž/Ù@ꇅšß@8q¼Æ¿äDFŽ¾¿á[©t0¿æ<ït—'¿çlãË¿ìK`†R"ø¿ïø¸®1×AGNbcu3FGL J1656.0+2044MG2 J165546+2043?ﱂHzRZ?€(ÏðØZ?ƒŸmáki'?€(ÏðØY?ïüptl?PûŒ¼Ê?<×\¦œ?PûŒ¼É?íëd"³£;? JŒQuãû?°¤ÛZbæ(? JŒQuãý?ïßS&¼1?_CRÝE½?pVzl¡çP?_CRÝE¼ÿ4FGL J1656.3-3301?Õ@ù	V4p@hH'ÓÀ8ç
ÜÒÔNÀ;)yÙ	ò@ÆGåœÒ^@Ršäó4@?º­j˜?Ót¯'@T+
oÆ@"4A{†¿Ïñ@õh¢¿ä^2.o¿ê¹Ë"}®W¿éY<a°@¿í-F¿×ñÄ¿ïÿηˆ—êAGNfsrq3FGL J1656.2-33032MASS J16561677-3302127?ï†Q¢Kûf?›֗'h_?Žk—m&¾?›֗'h_?ïT'¥!1¥?´bãÚáѳ?•o«[ÙËy?´bãÚáѳ?êùâÃ.­?® P©ôÅ?ÇøtóEJ?® P©ôÅ?î[B]z?–tf2Y®?ªKÚ.^n?–tf2Y®4FGL J1656.9-2010?ÞRo|àˆ@,5inX£À9j›‰]â3À;âxˆ§ÙÎ@ z—éJ?ýT¼ÕÞÄF?´³£(2ú?¸öª蟑@í^µ˜@J4Sï–P?‡µöØ %á?ïîÛJ>´¿á2"¢¶‡¿ÝœŠ$[©õ¿ÚºØƒA&¿àäõ¦n"AGNbll3FGL J1656.8-2010NVSS J165655-201056?ï÷´.§M«?I"ÿ}OÛ¸?P—¢±d¨‰?I"ÿ}OÛ­?ï·Åæ–.P?¢×Ö
¿q?'†Ztkï?¢×Ö
¿q?ïÐN×L§²?{#S\kâ?wؔY¬&Œ?{#S\ká?î‡î=¬·C?'¸Kðàg?§%4‹Å?'¸Kðàg4FGL J1657.0+6010¿¤7êf(ø@B´iaÃiwÀ:~oPóÇÀ<¥ôõ
¸@™'Ǿ,@cg]Ý*é?¼¥nS"Œ?¢ôšàÛ;i?äXy¾²Ø°@
	ú
å¿á†*Qb¿âO¾Ÿ !¿æïŽÎd|¿â°ô>«·S¿é¬¶ApØ¿ïð‰À]¨¨AGNfsrq3FGL J1656.9+6008RGB J1656+602?ïù"¤ ­²?A® ×)«?I­o}I4O?A® ×)«?ïýÿÞԋq?FØãMߓf?0	[¤s?FØãMߓv?ïä€Û×b¥?r]—…‹—?k$([¼?r]—…‹˜?ïô×Ï$/?C½4Uã$?VPa÷·¡i?C½4Uã4FGL J1657.7-6120¿¼š—®HÀ&¶"áÉ´À:ˆ™'6À;èZ§ìB´@>tà&ƾ@Nõ>M?ƛoG5ž?rŽÛ"T¥
?¢bÕã ÷@`Ü&$?Þ©'`ìÿȿꯍâ+XÉ¿çù¥=;ʱ¿Ù^–C"êf¿ë2ˆä?°¿€m»qAAGNbcuPMN J1657-6121?ï®
ø€Ú¿?'9¸ûBä??"}AßÉP'?'9¸ûBä>?ïû@#ˆ?aºY7'üÑ?Bÿs½ßä×?aºY7'üÕ?î£l·¿BV?™Ì3Œ,P?¥É4"Ú±?™Ì3Œ,R?ïåëÝ
8?WD¶‹¤¦?jæ"õÈ8?WD¶‹¤³4FGL J1657.7+4808?àI¨SaâÝ@C=½øôsÀ8'BhZ\mÀ;ü¯0ړ_@mE÷0"³@xÅÿS1Ö?¡"ßíª­?¼"N^‡Êº@	0¾
í)@q܂!ƒ?ßê
 AÿT¿âɱgì¿åù»þHoÛ¿ç	õíW†Ð¿è"9-H8¿ë3Ÿ¿£n…AGNfsrq3FGL J1657.7+48074C +48.41?ïè˜.¤?ÜQʺÖ?ggÑÿ[æ¼?ÜQʺÖ?ïðºOƒÏº?q0ä)?^‹`ø`Œ?q0ä*?ïÁM%œšô?'uXÚAê?Ym1²…^?'uXÚAê?ïݜtæÔ?[Ñ¢ç§Bñ?q1þŌ•1?[Ñ¢ç§Bî4FGL J1658.4+6150¿ìó^z@Buø"»ì«À;
ºª‹YeÀ<ÖFô@>#âÞ1#@ _¼(9Û?Çõ°[R;?¬`j_*™?á6É™"{@([DŸAN?ïaÜ>ñ§¿ç_d¥Ï2¿áȼœÓཿÔ|y"UÀQ¿ëþáòο¿ïì=ÆþAGNbll3FGL J1658.3+6149NVSS J165808+615001?ïå;ÖY}?eɛ§š•?jÄ)¦ñ'?eɛ§š•?ïù¶å±Ô`?d±&KV?I$i8®~B?d±&KS?dH;©?†,6¤Úî?‡æíñú?†,6¤Úì?ï¤ìõk¦Ì?p땠"ý^?†ÄÂ¥LË?p땠"ý_4FGL J1659.0+2627¿îct,Õ«f@AªÅO±À:±räùê<À<Q
¯ëëv@7;Îßw@'¤/?ÎÖç,õW?Ò(ŠBŽšã?úð"!'÷¿@ßëR?è0ál—¿èt9rèU¿èB¤À>I¿ìCŒFÊ¿¬¿æÑü·v#s?¹`4žWµAGNfsrq3FGL J1659.4+26314C +26.51?ïàŸ¨ðcS?v?7Uxž?o`Wœ¬ð?v?7Uxœ?ïåõ©2ó°?æ…âký?j
VÍO¨?æ…âký?îsŽÍ1‰?œ!ĤçL\?¨Ç,ï§l?œ!ĤçL]?ïh>€gIZ?'(éË?'ø/óÔÎ?'(éË4FGL J1659.7-3131?ís/¬3ô@Òø_øŽÀ9@Bæ.žÀ;'ëƒq9(@5ïù>@ðú#G,å?³ÊL¿Ì3J?µö<Ý«í.@=Õ%`â™@¤÷;
m?ë\ûÿr©¿ãt›Gï'ڿ收:º2¿Þo•¤—y"¿åeüH»Zµ¿ëÓŒÚnvAGNbcu3FGL J1659.7-3132NVSS J165949-313047?ïóÎçö»?U-' )¾æ?Yôb0Š0?U-' )¾ó?ïãùƒ {
?…/¶Òäë›?l|_"õ0?…/¶Òäëš?ï¾û›†VE?€¦'IYz?€Ajn¬?€¦'IY|?ïbŸG8µ=?{¥ÚNä6ê?"¬éXb?{¥ÚNä6ë4FGL J1700.0+6830?âC!3óå&@Aš¸¾øγÀ89FÍCëÀ;ׅJW<'@Â]ûu­@:>xá"?›Zm^Ó!?ºŽTììQø@ÙùŸ"®ž@TÖ}АQ¿Ú Ä܏û¿á1ìv¶?ÿåÚò)}¨¿æóe½Éû¿êÎ[–x¿é\°9ïAGNfsrq3FGL J1700.1+6829TXS 1700+685?ïç?š£(?c±Ì"õj—?hÀe\×ù£?c±Ì"õj™?ïí«ã4ú?t13FžÚë?bTË÷;?t13FžÚî?ï°VF
t?ƒÛmU^F?ƒên|œ¢ó?ƒÛmU^D?ïó¿O/³?Kež.OŸ?Yȁa ™[?Kež.O'4FGL J1701.0+6613¿ë,©÷,Õ@AÙR*o?SÀ9ì¸c­OÀ<y7ýO1@ë‡('çP@ÑBªŸ{?µ£*€ËÜ&?¨o¡"2
?í'Q;[÷@J¨¡tYn?·ä£Ù
¢Ö¿æêµ`I–Í¿è"œFó˜¿êƒCÿEÆ¿êí«i¥¶¿ïþ;âÐAGNbcu7C 1700+6616?ïüö?óîº?4UMáE¼T?8N`Š'¬?4UMáE¼y?ïü
Ï1/'?^•Ÿí??©†vƒqj?^•Ÿå?ïßå}Æ=?qŸk–Ò a?p
Aøà©?qŸk–Ò e?ïÚۈqvÿ?d#ˆK'h4?r';ÇDÇ?d#ˆK'h94FGL J1701.3+3956?؀vœu›@B¹Æ\pC_À:1!
;ÃÀ<Žgú»¡@ø˜¾ñî@2<ã¶^?ÆMO~˜a`?ʇò<ÈÞ+@£¼ÅîŒ:@GhÓ©	ú¿êZ…¢kÐ3¿Á‰¥…¶
¿áúâ‰Ít¿å–¸w«¿è×ãD8>¿ïú":½k0AGNbllB3 1659+399?ïHF'ùÚ?",<ƒ?–÷/§ˆÄ¼?",<"?ïù'Á<©Y?aÁ4Ã:?Iôû
Z–¸?aÁ4Ã<?íšUj?¥qde–o?³-WÏô¯z?¥qde–p?ïh¨¦&?zRæðsÊ>?'þ
ÿë;H?zRæðsÊ=4FGL J1701.7-5621?ï|
Æ=ºÀ!Œû¼¾bÀ:f/Ш# À;—Œ™¦@4›Jž´·@ >ê šª?È Br–K? "…`Q¤b?ܬ®^͕Ë@Zª=€¿?è›×âTžh?ïÙ_æÌR¿éùJn¹?¿è¸æ0K!g¿Î°Ý˜wÄ¿çë$ p¸ÐAGNbcuMRC 1657-562?ïP_%9Ð6?"âFÙ`Žž?•ôXÅùL?"âFÙ`ŽŸ?ïÆ"ND?"ÚñÁ»Ì?|îøØó^µ?"ÚñÁ»Ì?í6"2R–?¤´½E?¶NîmoU?¤´½E?ï&D%ÛHD?Â€KÂä?›7{D–÷ž?Â€KÂä4FGL J1702.2+2642¿åD
ŠÄ™C@A\‹ÁiÂ;À:"E>ÎqèÀ<ƒ:"ÀÅ@%|nWÌ@®M]€ä—?Àóîº2kb?¬±<Úý?íS?ˆÖÿ@	d\1"1}¿ïû>¤€?ïÿbì^bŒ¿ãrí]f¤¿áÌ@µÒµ¿ãˆpîèV¿ãÇ(žáŒAGNbllMG2 J170210+2643?ïþ¦Žò?!Aš"õåè?%—pߢ?!Aš"õål?ïý¤BŽ?JSìˆ*Ã?72ßÅë'/?JSìˆ*À?ïñjõ³×?a"°¾óX?]+è˜Qž?a"°¾ó[?ïìq]Aý?U6kp–õC?cŽø¢¾À?U6kp–õU4FGL J1702.6+3114¿ïü—káÚ@Aߓ‰µ À:R2#h»À<vòS4Z@ P‡[SÇ?üoøØ?¾Þsþªjw?³%ÏG{j?öh†>Þ@\'t/'?ïÿþBe«+¿ã¢UË
¯ì¿ÝþÄ+=›l¿Í¯u£ñp¿ÝÒõ:ªú¿âÁ<£AGNbll3FGL J1702.6+3116RX J1702.6+3115?ïÿ?N[ "?µʟ×?4›í™k?µʟ}?ïü!Œh€?Nǔ"ǁl?>÷㜻ÿj?Nǔ"ǁt?ïôþù©–¿?bUtq'ê?V¬Ò'H?bUtq'ñ?ïÄH°k Æ?bù'NÉm,?}Û§Êoœ¾?bù'NÉm,4FGL J1703.6-6213?Ǥnà‰£$À(â­ÄÉÉÀ8=֌i/oÀ;aª‡'§@G–¡—"Ý@áª$+Xs?¢þ\緊?ÃXeœ¼ä¢@Ê&½+.@Â*f…ðð?ïÿ«çy÷=¿áˆ¶‡¿åñ°F"HϿ婼'ì&.¿ë51ÛD^Õ¿ïÿø="ßEAGNfsrq3FGL J1703.6-6211MRC 1659-621?ï¹?^Eö=?0¡å>i	?°(n'q?0¡å>i?ïĵŸƒ†?Í8@Uˆå?}¥0x><ø?Í8@Uˆä?ìºÕÍœz?¨±Ûœgd6?º)Q—Ã'?¨±Ûœgd5?îcjfû
?–¡WJ¬}?©ÉYO'0?–¡WJ¬|4FGL J1704.1+7647¿á_ËW›@@1éÍ³}À9@UÁF‡À<M¼¢³Ï@¬ÙIÝė@S°ÄXŠ?§ŒàŸ©?‡–!jŠ?Üî~Î<9@­ÿ±%§Y¿ÔȨZ§–\¿ä_ÕÑXM¿èO/]e¶¾¿ã_lÂK¥¿éï81Ÿµ=¿ïW–Š •AGNbcu3FGL J1704.0+7646NVSS J170357+764611?ïûuòÊø~?:j{cŸp?B(4ÔF?:j{cŸp?ïþg˜)ô?EûéÈ­?.ن}`¸?Eûéȟ?ïà2þç´½?r"Vxªš?oÍKA¿?r"Vxªœ?ïÿÜ6²?I>ëëÚ8³>ñä¦à[w>ëëÚ=Á4FGL J1704.2+1234?ßò£2Æ@=f°¦üX¬À:UÎyu6äÀ<E¢Ä»†S@'ê0µÕd@1wðÚÉ?Â#•ÜJÄ?µ(õÂå?ñK
¥uoï@
jŸHZ6Ø?îÔÎÞõÄ=¿êè±d'z¿Ö{%¥«ö"¿ä¤5~ç煿Ý@ˆ[XÁ7¿ïÿï0l¯AGNbll3FGL J1704.1+1234NVSS J170409+123421?ïþéjü€?(òÜCùg ?.ÑiP7øD?(òÜCùg`?ïýÀšSÍ?Hé#în
¿?1ÿÃ-a"o?Hé#în
·?ïã"Ì¢×?t̐'¼p?llù3])?t̐'¼p
?ïðõ¤Ca?G~"ïöã‹?^à·y<
?G~"ïöãw4FGL J1704.5-0527¿æó°å˜ÿ@4ʂƒÓ^·À9Nµ×½Á—À;ΛâI5Ô@ =(Ɲ³°@Ga)Ä?®tÉUží쿕æ…ZZn?éά€§f@ý³¶P^'?Øø¾RW¿ã‹rX¿äÍhø¿Ûr£áq¿à×{ýQyð¿Í;;~AGNbll3FGL J1704.4-0528NVSS J170433-052839?ïø{vˆØå?F›­è~2?N%ܜmá?F›­è~(?ïû.¹Æëñ?Z~•â8ý­?CEäP:'?Z~•â8ýÈ?ïê®÷ÁÖ?mé¼·:¥A?eQ>)ã»?mé¼·:¥<?ïãFè_â?XÀêÀ'±÷?l¹ ãO?XÀêÀ'±õ4FGL J1705.0+7134¿é[ÖQ€v$@@úˆ?Õ%À;%J<d4À<ÍB=Jä@úCºÚ1@‹Ó"Qc ?Ë
ær@U?¿œ{Ì)8Þ?ò±‡Ìè{@]Ȑ'*?ïÒ(ŒD¿Ý*qB¸a[¿ã'<"pj¿à@ÛÈRé¿éÿ-!¡:x¿ïõc#»ÆëAGNbll3FGL J1705.5+7134GB6 J1704+7138?ïðþg®¦?`»©Ï?^0¢³× ?`»©Õ?ïý+¼¦Ýí?Q}Ó?6¢É–L?Q}Ó?ï´5š""??/ŸgAŸé?'ò™^÷pn?/ŸgAŸé?ïÃèÆ%?d˜0dþê?~v÷ík?d˜0dþâ4FGL J1705.4+5436?澖*ã½@B~¹ÃÌîÀ:Õ3YɟòÀ<΂€x`d@ <–Þ(i×?üeћh¦³?ÈzxJB?ÀFí9Ô·þ?ö HZå?ÿ{=pxãì¿ëÇퟫ+'¿ÖŠmÂ%S÷¿Þ]*¸b2¿Òg"ÄËL¿åè4ÂTxÓ¿ÕpÏØAGNbllNVSS J170520+543700?ïûsRŽ¯??/2Ï©?B2·ÑÅHî??/2ÏŠ?ïöۃJ—?lÚe'ŽðÓ?RHùkÖа?lÚe'ŽðÚ?ïêTtK­?mí
Eí?e«‹´èSŸ?mí
Eû?ïqkjÝ%{?yõÜtš?'Ò'¤[P¡?yõÜtšŸ4FGL J1705.5-7423¿í-—Û¡Ð-À3jâ¸Ç\KÀ;ÏO?ÙÀ<Û÷@=ݱ@#oÄ8(»`?ùŽ­\Äüõ?Æ_šYÝìÛ¿¬6^ø?çÐ3:}ª@'¹Ëé"¿ïþƒþý¡¿î¨§ž¿ô!?ïý6âjBê¿âÏ@Î&i¿åFß•e?ù<a°@AGNbll1RXS J170548.1-742240?ïÿ$tE'?&ÀHõ®?q~÷MÎ(?&ÀHõû?ïü@Ý{@r?dØ]ëæà?=ù%üp¸?dØ]ëæã?ïîî»ÿ¹?gq0O‡^æ?aDFå?gq0O‡^Û?ïêjûÛ8?fmÿö³£÷?e•÷$ÇÃ?fmÿö³£ý4FGL J1706.1+1000?ÊÅtyÒ)@;åƒjƒ,À:?Ò?ÓT¦À<ãAƒX@¬åm¶@³@ÔÜeÇ?ÉȹAՍ?Ã
é!›?õf"X@ÙÛÃO˿ךLGo'¿ãZÛ¿è…tžtG¿ì3l>¼¿ïé!ACAH¿îÃøþ.ÂAGNbcu3FGL J1705.5+0948NVSS J170556+100006?ïú¸üH[?EœÁWAu?G'ޛU?EœÁWA}?ïûÑx5?\dY""(?@ºç+ɚ?\dY"")?ï°î'¤Än?'d]ðh¡?ƒÄ[–Îär?'d]ðh¨?ïߟ{bl>?\'KÂ
BÖ?p0BNÉàÿ?\'KÂ
BÑ4FGL J1706.8+3004¿Ø"'‹õÐ@ALSóÀ;9ï•N±À<¥o@Î&@ŠM<žÁÍ@SÒDÛÒ#?ÅLLfn¿¡_w½Yoæ?ÜóD›:ƒŠ@ûÎíäJ¿ï5/øOó?ïþ¨Fۆ¤¿ì¢ì^b‹æ¿Ðì±#yó¿äC‹ƒS?³!Þ:øAGNbll87GB 170454.3+300758?ïôNnÈ®?TW©N%ô?Výc"n »?TW©N%ñ?ïüâý¦
K?V¡¨°ÂºÃ?8èÏ­­Š?V¡¨°ÂºÆ?ïÖOyv+?t4òSM	,?tØCDêtà?t4òSM	/?ïìÂfO"œ?UÍØد¹o?c=™°lc?UÍØد¹p4FGL J1706.9+4543¿ã«
3'ý@Bo.ßç[ÄÀ:¯¤Z½»¸À<_8ö@*‰¹QÅÅ@Ö#£s7?Ëÿ.^b6?¶~³Ë?é½ F@iùY¿Û^Þ&'d¿è-ÝvV¿æÐ
>Vý¾¿ë!°9ï¿ï÷á&öå¿ïÿöµšAGNfsrq4C +45.34?ïÿÌX\N>ùû.^3c>ùÓÑØÿž>ùû.^3Œ?ïü†ÎB6?^HÍr®Þ}?;ËñîHG?^HÍr®Þ|?ïé8¨ó?h1òhw¼?fÇúþW
?h1òhwÍ?ïïÌ*ÁÚ4?O[$­†º?`3Õ>%Ë'?O[$­†¶4FGL J1707.1-1931¿ïދ€kk@(ü)¥ë·À:ŽEîÑÀ<.·~†îœ@éûéd2@,p¼*¾?Êdk9‰äp?Øà۞KÛ@¥þ9Vbã@Õýê&$¿ï¿,Ñ?ïþÛ<Òf¿Þõt,öƒ¿á‹B=è¿ï›Ð`U*T¿ïÊ1¢ˆ.AGNbllPMN J1706-1932?½s7LU?µ¡Ï˜ìÉ?ì^™u_?µ¡Ï˜ìÉ?Ìk£Âx´×?Ð0{ÛhKA?èåaÒÊ?Ð0{ÛhKA?ÊiÓÑL?¶=""CôÉ?ée½Ë>K­?¶=""CôÇ?ËLª˜>"?²øJ,–?é,ÕYð^ü?²øJ,–4FGL J1707.5+1649?íø¡pÀ@>VÌ¢Ûa»À:4¿û-2À<L¡3ß@üÀ'a@DZ¢ãÅ7?¾¬W ùå?¾·ñH'$Þ@f´A»Œ3@
Ž~ZÎؖ?ïÿÔač¿âá',"³¿àêŽ^}
ó¿áŸv¼Ï)¿ë5â)>¿ßÙÙ«Ø`AGNfsrqMG1 J170732+1649?ïõ‹ej;–?p²RÜa«S?Té5+ˆÒf?p²RÜa«O?ïúƌ?\<ˆˆ¸?DåÏê®É?\<ˆˆµ?ïtPáó½ª?ŽX`çÉPÅ?'uãÁˆJÓ?ŽX`çÉPÂ?﬘ÍûXM?lõr¯/>?"Ù́)ì?lõr¯/?4FGL J1707.9+0016¿ÒïÙkG@6ü{þ~ÁÀ;‰‰¢À<D]­Z@¾@ Åå،s–@´ßbцp?Æy§¡D2࿔è:D')î?Бz{Ç »@þ=ìʙ?âziR©ñ¿Ø'-¿€Þã¿ëÁ
Áú᳿˗)gW}¿âòÅ_E4è¿Öi:@ԕAGNbcuNVSS J170744+001750?ïý‹,ëù?0ø³¾Ô¶?3¦˜§XIz?0ø³¾ÔË?ïþ¸úïU'?@El&¿?$pQ
¦Úõ?@El&¿?ïíéÈEÊ?jÔÙ{µš?bã7º4»?jÔÙ{µš	?ïþDη»?!CM5f?+³"NéÚ?!CM5|4FGL J1709.0-3525?}'¼5r'±@ŽÆ±À9ºâP3À;wjš¨@uZê²@f'amÙ!?ÑiIºß™?׺@Ù$@Y¾L×I(?ûÉTZ[:?ïß(Ÿ[zz¿æI]Áý¿ãù±œÅž¿çޘÜÛ7Ê¿êMDƒ½¿æóï»åüAGNbcuTXS 1705-353?×àÉ/l#?Ëú´XÔúŸ?䏛hIï?Ëú´XÔú ?Ö
"Þ7`¾?ÒÙ£"÷Î?äú½äO¡?ÒÙ£"÷Î?Ø»xî.ôá?¸I}!ó?ã¢Cˆè…?¸I}!ó?Ç¥©«?©Ç噾7Ö?ê¾Õ•?º?©Ç噾7Ö4FGL J1709.7+4318?ç÷LÔi‰Ü@BÆâ¨eÀ8dVôÙ[À;ÑLF)¯ý@¶Ò«@Å}?Æ¿m? µ"â>?¸¦‹€¸]e@ŸAò×s@nE­ß â?ï¡Ä«–`¿ß!æúËb¿¿åƒC…¶ä¿äÓkL4"¿ér†áa¯¿çƒÐ¸ò$AGNfsrq3FGL J1709.6+4318B3 1708+433?ïöÀenW?L"2¬IŒï?R5#ÉP
?L"2¬IŒí?ïó¶¯=@?t½i@ǒ¤?X'¡…×??t½i@ǒ¤?ï­_)¹ì;?…@¿Òã?"¨5'"ñŒ?…@¿Òã?ïÿ<ÂÊÛ?î–wÓK?g½æ¤¶<?î–wÑí4FGL J1710.1-2030¿ì5»ÚsÁ@&°Z-rÿÒÀ:¥P¥4À<(äSÒ,@bBÁñ@ÐAÌS*?Ëü¨>O?×éw}e"@o?Rü&W@M™¢Rû¥?ïû´a"ñ¿åd8>4îõ¿ÈFû&§^©¿çŽâá·ª¿æ÷mT—1
¿ïÿW~lªAGNbcu1FGL J1709.8-2026TXS 1707-204?é˱µÞèæ?Ä°äh' ?ÈÑ9("\j?Ä°äh' ?àÍV_4¶Ç?Ò£›sùÚ?ÞeSA–'s?Ò£›sùÚ?å­Ä¯(,?¶«]ã؟?Ô¤v¡¯ï§?¶«]ã؟?àÊø©¢?µÚJòÄ?ßÁÂj¬¹?µÚJòÄ4FGL J1710.3-3943?Áødç:Z?¦Bî"n%3À8@‹áJÀ9îÐè»?Ý@ܶlŽ@Ásûz_B?ºÉ³<ØÎc?Òê©â<Á@¶8ݗl@–f‹û r?ï¯Çˆp|?€œ ½­Ó–¿â‡ÐCyÒ¿èöN¦V@¿ïi˜¾&A¿ðAGNbcuGPSR 347.050+0.041?H‰Î…JÈq?D"Âáœ?ïù݌^­N?D"Âáœ?y›b·O'?.œý7þk?ïÌÉ:'`Ý?.œý7þl?"¬(˜Äòb?ux%¿sX?ï­O]œì5?ux%¿sb?`Í9XHîf?Mprk`x?ïï2Ƨ·?Mprk`y4FGL J1711.1-4600c¿íEýœ%W½ÀIZ¼äø=À9œR3©z¸À:µs¯ûî@ÿö¿ºj @i½@gÏ?ךŒàŸ?םŸQ>Œ@ÇOšr®@®ÞzIG¿à7(áÀ?ïÿÕ"[ʁ¿ê­ÂC±Ü¿èV° Ï/¿ïîõÁ2e?ï
•ö]AGNbcuAT20G J171106-4552548?æ>kÉýÑç?ё­ž1%?Ӄ(l\3?ё­ž1%?â"ã^›U(?ՋÜD½?Ûº9BÉU¯?ՋÜD½?ÜVk@9´?µÐakã?áôÔÊ_ã'?µÐakâ?Àb"mKxe?¶°ñ-O$?ëç[$­!å?¶°ñ-O%4FGL J1711.6-5027?åF/ÀWbÀ؏>ÕÀ9Z`ȗ³æÀ;mcr–'@BDmÃ'@WS£ìó?º S7
?³'T®ƒ
·?øÂ+‰Æ@t&µ÷HK?µëî>ü-ý¿Û2¼`¦¿ê©ãÉh">¿â'¾@—õ«¿îo݈†Í?Áê}ø(p7AGNbcu3FGL J1711.5-5029PMN J1711-5028?ï?íV+?›êÇ3sÎ?˜LU:ž{?›êÇ3sÎ?ïÆHk¤¨‡?¢¯Í ª?|ÛÊ-«½?¢¯Í «?îÌ9Yx?ŸÒUÑ&Ë?®s<jn؇?ŸÒUÑ&É?î÷8KüÐ??Š†>	£›œ? Œ{@2ü?Š†>	£›œ4FGL J1712.5-3142¿Ô#ÓM‡f?@«½À9ÁöBçÜÀ;2H˜F@®Ÿ]'ùC@be+ÓÃ?Ñ|Òì™q?ØѡȽ@²q¼Û¾?þœyGêz?îÄ!ÝËLÅ¿ÔfˆË<¨¿ê§(-E³h¿å¼þùoÿç‹5ó×ӑ¿ïÿõ^'AGNbcuNVSS J171309-313912?ÛÖ«­ëÐ?Ñ[M)+›‡?âª)
{—?Ñ[M)+›‡?ÐßHàl½?ξ"M+'Y?ç[÷É¡?ξ"M+'Y?ÚSµR~ñu?¼¥ýٟj?âÖ%VÀ‡E?¼¥ýٟj?ÆØ2'~?­K¤T¦M?êIóyŸ¡?­K¤T¦L4FGL J1712.7+2932¿Äøà¤ò£'@@t`$-À:HOžÀ<e$îÌÑÕ@ ˜V]¯³Œ?ümfL~?½
ãÉ­?ª$÷A{±?𨯠Ä?õeª^Ôê¿ÚIËÛ¶µ¿áh¼""Õ¿àXa@ß¿Þ~+ÿã$¨¿ÉI"ƒ\ì?¿Ú6›¦AGNbll3FGL J1712.6+2932RX J1712.8+2931?ïõþ0§IÝ?Q¹IÝÙàã?Tž±lEò?Q¹IÝÙàç?ïÙRÐé}K?ž"&ðÕ.‡?sV—‹AZ"?ž"&ðÕ.‡?ï݁ö‹·Ö?v[j¶g|c?q?º$|?v[j¶g|[?îÉ«ÊC™?ŽP{Cq}g?£eC[σ?ŽP{Cq}f4FGL J1713.7+8844¿ä1»i{ $@;¤ß&k¤"À;Œ`b@føÀ<ìXJCðñ@!aTБÓR?ûNB¸â4=?Ðë}&œKü?Å4á^)V?öžÜd…@Ó~Ì
à¿ïÿÔÌuŽø?ïÿ®XëT¿ÅZF@+>¿¹\èä/"î¿áŠ!¡»Q$¿à…ïbùÊ\AGNbcu3FGL J1711.6+8846NVSS J171602+884416?ïüädìâÁ?3ª‹'>?8Üؘéñc?3ª‹'?ïü\碔É?VüÙ uw"?=ÂëYÃb?VüÙ uw+?ïÛ'هµÊ?r••—m$?rl<%q?r••—m&?ïÍ ò·µ¯?fÒZæö?yo†¤%(]?fÒZæù4FGL J1714.0-2029¿ïò½¢÷@%4f+®´À:N{.t‡'À<
-€kË@#ÿåSƒ?ùµ(Ö¸ÞÙ?¾è(råЪ?Žtøì³?Òñ£[dT¾@	¼IGǕ¿ïÌR>[î?ïýð@o[Ø?¡K'_¯ª¿Û¼J~Sm¿ÑMR-Ê=¦¿Ê÷µP-ëAGNbcu3FGL J1714.1-20291RXS J171405.2-202747?ïÿ\d"š³?À3®ä?smŒ©ÁÝ?À3®ã?ïòM'ʨ?"âW?[Õdúj­Ã?"âS?ïêèQ¾
c?kˇv›Í—?e®Aò›Ð?kˇv›Í'?ïùC\[?BŦ˜`!›?Jòú–s?BŦ˜`!4FGL J1715.0+2616¿Ðªb'`@?×a»úìÀ;ú61ëÀ<uÌÆ폻@÷ݜ¨Ã@y'½µÕ?̳€u†>ô?¦6ÌoÚ®b?ÔÏí~<Q@j#¹?£R~ÁÀÃï¿ä±À¢¿äþh›Œ¹¿â-t½l1¬¿ïþ*½ÃÅg?ïæ?šIÂÂAGNbcuMG2 J171454+2614?ïñå>LÎ:?W¬œÁHW?\5ƒfc‹?W¬œÁHY?ïöüºpHš?z"Fí?R‹nˈ?z"Fí	?ï¹2½¥?èÚȨ̀(?½3z–‰?èÚȨ̀ ?ïéï%×_??WE"e
ä?fÚ( ¿Þ?WE"e
î4FGL J1715.4-4025?ÁÕ­QYGÀ¿ò"ãw3=DÀ9Øc—À:ð}e†l–@ x>fB)E@ð	yü?À¦Th-á?·vÀіá?ø ­Ú™>*@jÆ?ïþü—åº?íØ@|g°¿å†\Û£)e¿Û‡ôU§ÒB¿å"i£ÙŽ¿é»ÃŽAGNbcu3FGL J1715.4-4028PMN J1715-4025?ïÝý¤½ŒÓ?zUe€!?q-¡9–»?zUe€"?îÉ_ÿeÅ?¿¯R«"ô¦?£j 	£É?¿¯R«"ô¦?íeoE­îŸ?«àTÈ^i1?´Ô…Ґ‹?«àTÈ^i2?íým‡"?¡Üâ˜V5ä?³ð"Ã_X?¡Üâ˜V5ä4FGL J1715.8+2151?íÎGfB¶@>HèÙrÍ}À;!•¥ïrÀ<Ž*pìÒ&@ó}Ë$@–U&£ø?ÍÕLù	ð?²8ÀxÅR?ã1&¹@(@"Üç÷öq¿ÆU±7pÉ¿æm¢À^ÕM¿à¶8 WäC¿èRˆÎp:û¿Í÷¤¼¸W ¿ï÷ÔCédAGNfsrqB2 1714+21?ïô´½l?Rb¾æsŽ?V–…'×Ûh?Rb¾æs?ïü'oÏ0*?[¶Äx©?;l†~¹s?[¶Äx©?ï¾^£G?~Ö·gÊû?€hxü×.|?~Ö·gÊû?ïà!_ޔ?]…;.Ë?oÞ ù!j¦?]…;.Ë4FGL J1716.1+6836?ÓkZ€°Ù@@áOKD¢À9°›±¡ÎÀ<qD…kl@$´o#@ðçä€G¹?°Od´Ëy?‡Ç8ä"(õ?ÕòoÀ@X%åí°?¼]ø®§ó¤¿â'f$!Gx¿ç2bo¶Ç¿álÁŸG.¿è7®ø¦ok¿áº>À//˜AGNfsrq3FGL J1715.7+6837S4 1716+68?ïû9Gf>î?8SÏ:·ó?CâgHL?8SÏ:·ô?ïþ|ò!·??å*˜´µœ?(0Ýï´§c??å*˜´µ©?ïç{}«·?q=k$²W?h"'üTHX?q=k$²P?ïÿD^A?
†Üa]&?|7ÝíL?
†Üa\'4FGL J1716.3-3421?ïhÊĉŠ@ݨ!ò™À9X™I—À:½r`o¬`@ZO+â1@¶Ú@¨?Ä'îÆò˜8?ÎÅ3æ·Yž@v§&J@¥Xz—?ïԋ/Ÿ*¿çÇb\«¿ÙÏ QC¿r¿å\½p8w@¿éÄ
¼¤¡¿ïý"#–]AGNbcuTXS 1713-342?Õ{WòW$?ÊúªîÿV?åBTñÔo?ÊúªîÿV?Ûü"7êvû?Õ$Iø¿¼?â½ä
ă?Õ$Iø¿¼?á4¦'
#?¶úò'ºÔ;?ݖ³Äûåº?¶úò'ºÔ=?árƒ'°
x?¸` ¹jr?Ýøڟå?¸` ¹jq4FGL J1716.3+3434?¡˜Ù4þ/@@Òb^™éKÀ;·ÀÌ
Š,À=yÚ6AÛm@[ N@†A­
ë?Ó¡Fnªƒ?ïþ@_‰Ó@9¥e¶š?þïΔ£º¿ïëiÀú)?ïÿæ4|ßO¿Ïàœøɪٿì¬Ù¢s1ü¿éæràÈ,T¿ïVqáÄ«–AGNbcuFIRST J171642.1+343856?¹}¨XÁtû?Â
nÙë¿?ìÐJôçÑ`?Â
nÙë¿?±òmˆ÷?©ä¥~?íÁ²MÿNá?©ä¥?ǧžJ'&?³eZ®ñ-?êm_vy?³eZ®ñ-?™ª²Ò$?'¤óS`ð«?ï2ªioß?'¤óS`ð«4FGL J1716.6-6707¿ÛªÅ0®Ü´À0Q€¡{kÀ;<MI^ïÀ<|ók@•±êk@<î?äž?Í/d\ m? j‹Üdî?Ö²Üá—à?þÌmŽÎºc¿ÒFr©jÈ¿ãIÒ±é¿èg
À²ã¿Ä˜†t¿ì!€ƒH¿ïÿîÝÃÀ	AGNbcuPKS 1711-670?ïöúˤÓ?J¤~ìý0t?R
h·àVƒ?J¤~ìý0w?ïâ¸"ÿp¼?‰0¦Ž~?mGݏC?‰0¦Ž}?ï¬Å÷^~»?ƒíQ¦7'C?"΂(`QÂ?ƒíQ¦7'G?ïÇ4=£•I?h§e
ŠíI?|eá.5[r?h§e
ŠíH4FGL J1717.3-6045¿íòMïMÀ)ížbV6mÀ:ïdDM6êÀ<•—rwí@6ƒºŠ*@mUhƓ?ːЇÂV§?ܚoÂۇP@=TT+
@jŒ¢:R¿ïð‹ž.SÐ?ïÂ{ƒ€¿ÖŸ§z­Æ!¿æ=í¡X«¿íĜý|B¿ïÿü¿ÙŸCAGNbcuPMN J1716-6045?ê£+œþ?Âª¨€™?ÅsïSµŒ?Âª¨€™?çÿ²ŠŒ_?ÑO/A´ý–?ÑÀšêçB?ÑO/A´ý–?àe¬þB<Ñ?½ÏUµÌÆ?ß4¦{†[?½ÏUµÌÆ?â'üóV÷?¹5ÏUçÿÁ?ÚÝÖR?¹5ÏUçÿÂ4FGL J1717.5-8114¿é]B‰À7^'¸#È\À:–@
²
ªÀ<iqDæ¹Þ@×`]bÝ@ÈCæߞ?À»¡VQp`?Ž¥vLJ"?Ììa<°à]@íBDH.m¿é
Ï@Åm¿Ù́»¬i¿ä I·¿à^^…¿áü¦¯+Ò¿ã!R•Ï	¾AGNbll3FGL J1716.7-81121RXS J171712.6-811501?ïöb?¹?LÖõ÷P›Ÿ?S;ÐÅØ?LÖõ÷P›Ç?ïþ‡ÕOö?KÀðýíÆm?.''«­'?KÀðýíÆz?ïç\˜E?q,«Åò¤Û?h£÷gþ»š?q,«Åò¤à?ïî °¼¥?PÓC$€ÈÖ?a_OîC\
?PÓC$€ÈÝ4FGL J1717.5-3342?är‰leê:@'ô}ë¾*À8:¯^&üÄÀ:[";"*Å@#ý:¨Èa@dc!7ˆ-?±LžŒˆ?Ã`à?›Ku@U£ãŸw)@4´g¦,?Ð87~òNg¿àÁQ'Ò­¿æl«ÅHg¿åðQ£"î¿ì›]"°§¿ã‹Ú"5¬ŠAGNbll3FGL J1717.8-3342TXS 1714-336?ë踠1(?·¤nî×~¶?À]³;e?·¤nî×~¶?ï²¥êlhd?¥
VÌ܅?ƒV…dåç?¥
VÌ܅?ç…?ò¬þï?³…˜—(~W?Ðõ€¦#?³…˜—(~W?ïZý)ëþ??‡"Dì\¹:?" Z€8?‡"Dì\¹;4FGL J1717.6-5154?²Q†§ÁÚÀ "ön†ÆÀ9r"áÉ´À;x"íˆ.7@šU'þ@%!4y?½nýùëi?ؼ‹ ¯ø×@¯œ…×E@ 	%m¢Æ?ïû—áÂA¿ÙßND0±y¿çœ/`•Áô¿èÎ,~
L¿ï\˜AÒ¿ïš@¨f¼AGNfsrq3FGL J1717.4-5157PMN J1717-5155?ìJ-Œ¶½Å?¶‰E!»?½®"šJÙ?¶‰E!»?ïðþú±"?qáŸPŪ?^
ðÔÀ?qáŸPÅ­?äM–ÿ8Ìd?µF?zîy?×dÒŽg7?µF?zîz?ï†gIæ?}ÎvžNç?Žf9¸-†¼?}ÎvžNå4FGL J1718.0-3055¿ïí䟎§:@7%€ÃÿÀ9<,†pÈÀ;Eˆ×ªva@–]Z#7@	•övê?º¿Œƒn_?µÎ–?`×Ë?û¼µ'•@ø§üaæ?ï}!"Î~~¿Ý]ÅB"пèw¦×o¾¿Ý*Ü·ü[0¿ç#ÑÌk¿çx×ì;AGNbcu3FGL J1718.1-3056PMN J1718-3056?ïDçï`Ëa?›;mCc;?—cæ"Ä?›;mCc;?쇎gþÒ?Ǧ´>mE?»ÇûŒÀ	l?Ǧ´>mE?î0à¨JL?¢zôSPJ¼?¬ñõ{^û%?¢zôSPJ¼?ë‹Ä·b Š?¥ƒ|ÚçÕ?ÁÐí"w}Ø?¥ƒ|ÚçÕ4FGL J1719.2+1745¿ÐH£>V¾T@<†`ÔÀ8®j}L\À;®z¯É‡@B.'åue?ÿwÓv4:?¤ô^¿±Žá?¸??ŸÁëŒ@_e©Oð@"µçØí?ÐÞ;Ÿ"X¸¿Üÿ"Év7¿à!,jº¿àÑÍmÜ|¿âÎHÍÏ+L¿èÛÑLŽNAGNbll3FGL J1719.2+1744PKS 1717+177?ïý^,VSÖ?,ºî':š?5MaXÂ?,ºî':i?ï÷†O|>s?c:"3™â²?Póaƒz?c:"3™â®?﹑'M'æ?…âp^l?›¶,¶\?…âp^l?ïÿڅíEµ>æi|¼<¥ì>ò½	]$áˆ>æi|¼<£Þ4FGL J1719.3+1205¿å+ìW'ß@9ØÈÿ¸²dÀ:Lí=…œÀ<4•äÙ3
@!; ¨×z?þ"ÑH\$?»1)ÑW÷¿™I#W›?àä†&ö@RgÎÆL*¿Ò亼)¿è	ØÆÖÇ¿ã9Pïܹ¿ÕõúX R†¿Ý±ª|ÀÅØ¿ÂlF9Ë'ÜAGNbcu3FGL J1719.3+120687GB 171701.0+121016?ïýAÖ¼9(?/$™»œ4)?5ñJ6Â?/$™»œ4?ïýà\%EŒ?H	¡b†Ú?0ýÕÓª?H	¡b†Û?ïøQ_«Ûq?_"µ€Á½?NºP'8f?_"µ€Á½?ïð7^ÞÕ<?LòÍä?_'BBU‹n?LòÍð4FGL J1720.0-5101?ë‰L
©'À‰êpKÂÀ:^Òn¦À;~1ôo@ڋIõ—q@À¹Ü/@_?ä/IŒ;?è?üÚ±'Þ@ g–@ý¦oëË@?ï8S~,UÉ¿ájzÈ:£¿éŽ¬ l¿î`ñ²_c¿Ûn€m¤?Vérí)ÛéAGNbcuPMN J1721-5055?è ˜×|?Ñ>è:/5?Ï©}œ¢?Ñ>è:/5?Ý|¦·Úú?Õ3Ϭò<?áA¬±$ƒ?Õ3Ϭò<?áWíU¾?¼Ó;ýR݆?ÝãP%Uʄ?¼Ó;ýR݆?ϐاWæF?ÄÙÉÄéyG?èÉÖ*n?ÄÙÉÄéyG4FGL J1720.2+3824?ïöù# -›@@̴ἩÀ:¨–ùݧÀ<pÍ_™Ä@bl¤CÔ@͘ÚVù?Äíañ34?µ>M˜-…?é·ýgŸKŠ@Ìٌù£¿âSQ¶«ù¿ÄGRºb¿ê"'úð̆¿éâi·S¾Ä¿Ò+A!]s¿ïûÜàSúAGNbcuSDSS J172010.33+382556.1?ïڄÞþý?w­Z±­>³?r½€ÿ'9?w­Z±­>³?ïú҂;7†?b"~6»3µ?Dµ÷!ìº?b"~6»3º?îàŸSÀëØ?•j€Ó
DÈ?¡ö
ÃñB¡?•j€Ó
DÉ?ïÕINE?e&Ej°	?uz@[XÝ¢?e&Ej°4FGL J1722.6+6104¿â­ÏÝC>ò@Ap\‰mÒÀ:2ì|•|ÔÀ<WÄ/oYT@n
I¯÷@š%™í|?¼•p•x?¶7¸¨þfx?õPû«©@8"XŒÞö?·äùibð¿è™‡+¿é‹K¿ì&+¾ß¿è!p}–ƒ»¿ðAGNfsrq3FGL J1722.7+6104GB6 J1722+6105?ïþÓÞâÈ?!ó¤x½‡?"Â߃`?!ó¤x½å?ïý~ð+Ø?J¨¨—Õ
»?4æ¡7Ž?J¨¨—Õ
®?ïмÄÐ[?~Sa†ÃD;?wó!—Ò£?~Sa†ÃD;?ïö†³rGÆ?C¿¢@7?Rò™pt¼?C¿¢@!4FGL J1722.7+1014?æ7ßµ@8M¤-fkÀ8ù˜zµ¨ÄÀ;ãn)©G@Z×^K9å@qû9Ç¢?ªc,u)?ªÙ¿4¢Ž?þáDŽO¹@!O[?ʋîظh¿á!—à¿ä99±Êé¿âwÜ{~¿å¾´`šI˜¿âgƃ°AGNfsrq3FGL J1722.7+1014TXS 1720+102?ïû}¦?Ò?;švÔ!Ñ?AÂ	g¼ö?;švÔ!ë?ïüÉA+£?S¿;Œj?9µóö¢ç-?S¿;Œj!?ïނ©>'µ?uV¯ÿé?p¾«`ì%:?uV¯ÿß?ïüñìÌ?0š–‰(ùo??@p›¡±?0š–‰(ùN4FGL J1723.6-7714?¨ü:–‡×À5Ë6žË2À8J¾*ršQÀ;Ÿ0µªq@¼n<c@t@ylÓh?Ÿ¡"
R%?¹?æàIV`@4·õ¥3+@
5"Š¶Ó?·ßW=ÿj¿á&B‰èK®¿ãX—Ü*7â¿ä'ô¦/ª¿é±k«¦·¿â.•3ÙKAGNbcu3FGL J1723.7-7713PKS 1716-771?ïõ·áäÄ>?Tô £].?T<6w††?Tô £]?ïùà[œ…'?U›C‹"a»?H~'ëbÉ?U›C‹"a½?ï^†Ãl~1?'}°ýºu?"/''p9Þ?'}°ýºv?ïþKï¤?)%•¸?+HÊ£?)%•¹4FGL J1724.1+3304?ïEÎñ;¸â@?»XK±À;$Ÿ¹šÀ<¿Áõv@ÄÑÞ¯xS@ȝ»gI»?Á××WjJ!¿µE@¦ä/ë?ï$8ž×ñï@½´«î±?èÚ>Oq¿î|b¡µÇοÇY¨‡s&¿Ó³ä¡Q¿á'óU͒¿Þj~yÊAGNfsrqB2 1722+33?ïúN2j?Be[›lS?GöÇ6Wšõ?Be[›la?ïþ¹_ÄÑ??H'ÀDÖ¨?$nš²ñ??H'ÀDÖs?ïß3®û'ê?|ÃA°¦±?pf('>‹/?|ÃA°¦µ?ïèW¢Þ?Sƒ~U!ˆ;?gî¨]í#?Sƒ~U!ˆ54FGL J1724.2+4005¿ßTãK˜€@@'dobÀ9biAâù_À<RS‰êÐ@fëÇc×@§Ös>»ý?°ô¤9/Ì?ÁÔÀa.™@döÄíÛ:@Ž¦‡é˜à?'M
`!)¿â~€Ǒ$¿æ@&`¼Ù:¿ç—áìèì`æʤԿïýø‰9™AGNfsrq3FGL J1723.9+4004S4 1722+40?ïó׌¨«?SåB`?XPtÊ®«Å?SåBZ?ïû/5§_7?ZN¡Ùð•?CC)bƒ&V?ZN¡Ùð?ïŸ
¯¡Ñ|?IwÍ?ˆ=T‹ Õ?IwÌ?ïþè]Ÿ,+?ô
¥¯ZB?!z&
=V<?ô
¥¯Z4FGL J1724.2-6501?îÙW	]LÀ/Ç$ p¸ÐÀ:¹n$ É9À<DçԐ@8O§³
@ê/~r̦?ÅÕ^fWM?£GPCۄ?Ý܏¸oH?÷<í–ÆÖi?مâ,°b3¿ê~íEé]¿èS¤Wb½d¿âr‡ÂÀð¿ä÷ÞþþxA¿ï뒠+.,AGNrdgNGC 6328?ïô!N9ê°?Vû ¬ö—J?W½cŒ*žÆ?Vû ¬ö—K?ïYDÿ‡Åí?¥¯bz–?"×`B9?¥¯bz–?¯Azþ?‡Å?Ývþä?"/¡@'?‡Å?Ývþä?îÕFdw?‹º &QY"?¢«™¿Þx–?‹º &QY'4FGL J1724.9+7654¿ÒãÀš,Ê@?9¦ç_ö
À:¥ìeïH"À<^n£KÊ@¡@-lŸ»@¦;îך?Å0‹x™™Å?Š,†==ŀ?Â{R'L@	1‰èv¡r¿Ö5²ÿÇ ¿ç$w®G¿é¢
qÊÛ¿å`ø0'æ¿ãÔÄ}ròf¿ïÿïn¸D€AGNfsrqS5 1726+76?ïþ.Qù0?,MÃâîÛd?-àfüí(?,MÃâîÛR?ïþ»\ã2?=Ê£
š¦‹?$J8Ìêí?=Ê£
š¦©?ïä=d`v4?nj<´÷Ìz?k›Ÿ‰Íd?nj<´÷Ìk?ïú$ýPˆQ?6|Å®ö‹ä?Gl
½Þ½?6|Å®öŒ
4FGL J1725.0+1152¿í"éÿÑ@8yLýÔ»À7éÇ88U²À;*µ[–ÿ‹@°\ô͜Ö?ü@—"ìck?ŸÃËØlNn?®}£;P[@Öâdä†'@
s—ý7N?暴f¶î>¿ÝЎÃ|Áò¿ÜWí'?2E¿×QDX­¿à"$݅Û¿ÝÃÎ ‰ãCAGNbll3FGL J1725.0+11521H 1720+117?ïü«1%¨õ?5g2%ô¨?:¦vÒ¸a€?5g2%ô?ïµ@á¹?›eߙU?'¯ÛùG'?›eߙU?0ÝA?8iÂЇË?‹R3È»¯÷?8iÂЇÎ?î°&£¼Z?"îg»(%?®tý•Ä:d?"îg»(%4FGL J1725.4+5254?ƛÿ¥'@A
ïܜM©À;°£µ|N/À<Ó¿jäz@ ¬Í÷ó—@"0Ÿ<¦?")JÒ¿¶9&ôŸ?õe=ð%—@ŒUðLƒ¼?åãÉjÉø¿ê¶u¨"ÉY¿æ­}±Ü†~¿ãÅ6jö ¿Ø6]_+´¿ÆŽån.\AGNbcuRX J1725.3+5255?ïód¤E?LqOM®b?Y6·Õuû?LqOM®X?ïü ´DÝõ?QüAV"?:ú]ÙN©?QüAVž?ïîÛ>ÃÃ?f@›j(Ýn?a$Á<è<…?f@›j(Ýe?ïÞ&¤">ÿ?aˆl¯=Ü?pì­µàƒ?aˆl¯=Ú4FGL J1725.5+5851?ì¦ié®@@üšõºÀ9ó+w}À<'\ä¥6@O²×-Mì@g­Ãó	w?±ñOŽÀ?žmã;åŒ?ë?N_¤@-2¢""ø¿àžóu®¿ácAM¨)¿äļþ"°.¿Ý»¹^Û؃¿ç
ŸàÛwŠ¿áM20±ÏAGNbll3FGL J1725.3+58537C 1724+5854?ïýûŽàý?%é.bzÆ?0#ˆÿ ×?%é.b{?ïþ7YÌR0?F÷‡Žm&
?,Šc:Ýl?F÷‡Žm&?ïóˤÓ´?fu#0uLè?Xh·ÖX—¤?fu#0uLï?ïýùþ7QÍ?"¢£ò««¶?00Eq‹½?"¢£ò««y4FGL J1727.2+0644¿ÞàŠ†ë@5ÇÛLÂPrÀ:†R{ÍÖ¸À;ݗkÖ@ޛÇÇ)u@—¬úŸmï?ßB"úùZõ?åðBrÁ>?ÿË.LC¥q@	$á‹Ë¥°?ï/›™N?¿Ýsdѐ׿ëmµz °¿ê3­Á錄ïÿý¥\Æ?Ü×æ¼5CAGNbcu3FGL J1727.4+0634NVSS J172720+064123?îùT fá?­ŽõÏÙ,¾? jµÿù'ð?­ŽõÏÙ,¾?îàª]l¬s?¶Ha²c)1?¡õZ)58Í?¶Ha²c)0?ëõBʋ:Ï?§+ݼx.?À*ôÕÓÊ?§+ݼx0?îÍÓÐi
é?"ªz¨À¤ü?£"ÂùoQ€?"ªz¨À¤ü4FGL J1727.4+4530¿å±P"W÷u@@¥‡+À8qq¡-ÒÀ;ÿ+Ü&Üä@Jž5àŒ@'eŸ—
? p·ß;¢?µq"Q³ÑÔ@?Ø2\@|Ë¢Ö.J¿È+ç—rx¿ãšG>'òŽ¿æýdQµ¿æ­ÞÎW¿ë#Ÿa¯g¿ïÿÍ'ý AGNfsrq3FGL J1727.1+4531S4 1726+45?ïükǦ%0?2Ñ÷›È7?<¡ÂÎֆ­?2Ñ÷›È.?ïù\ý9>?]|zW¡¾û?K¦ŒX?]|zW¡¾þ?ïÇéÛʨ?€ Ý:ÿ?|«óS?€ Ý:ÿ?ïýß
÷Ƈ?"®:1>?1AËؘ?"®:1b4FGL J1727.9-0654¿ÝÇTÛCŸ‡@. ½ì_9KÀ:AíHmÀ;Œ¿®Xë@±F ù4_@Õ%t.?Ë*"<m2?ĈSvÀ5?ú§ÇúÕô"@V½sé[Ï?ïýª R¿æ‰ùž<°¿ã~ÊuÚw°¿å¢>ƒÉN¿ïõ}$îÌÒ¿ïë%@@AGNbcu3FGL J1727.6-0654PKS 1725-06?íÿìsHm?´¯ÎD??°œe¼—õ?´¯ÎD??éÕ5è)Y?ɹž²4ú]?È«(_Z›"?ɹž²4ú]?é"¨§?¶Ažä@:?Ëó±ïõ]d?¶Ažä@<?è½3.¥¾Á?«,øMD@`?Í3Eiü?«,øMD@`4FGL J1728.0+1216¿îÜ(ê@7ùSÞ¤e¥À9,ÂËÂÀ;Ì4–	Â!@¤é
ìî@qÈâ\?±\Á! ?·›‹¡´EA@³¼?¶Ï5@€'4Í<3¿à#Cf‡–¿Þ
D<œ¿æcˆ€l¡ê¿æk:ÁG¦¿êœ€iFëw¿×ú ø2¬AGNfsrq3FGL J1728.0+1217PKS 1725+123?ï÷KÆ®:1?L¡Û'z?Qhr£‹›Ã?L¡Û'yþ?ïùÙ Œëy?f-í´™°?H™}ÌRþ?f-í´™³?ï@0Ž?'&	I)ú!?—ùÿN<`5?'&	I)ú ?ïíÏäå_?R^ß®,ØØ?bë0¢u?R^ß®,ØÕ4FGL J1728.3+5013¿»f[æ‡-@@ÄÁæ¯ÍÀ8'û¡ÌnÀ;·–5df@ Ïÿ1N?ü%Ê_4Bþ?Ÿûß=#?ˆæ2	Μ?ê{`ž{V@Â
Җæ6¿äŒšþ§±¿à:þƒ©¿ßý‡[ח¿ÐþD4ã¿ßlL#Å&¿ÒèoÀ';¯AGNbll3FGL J1728.3+5013I Zw 187?ïÿBjZ«Ñ?R÷EFÏ?²´ª…üÇ?R÷EF¢?ïý¬NØÄö?G6Mþb,?2‰9ØN¢?G6Mþb,?ïå¦ÇE´?u—ÿ¢«¨û?jY8ºbL?u—ÿ¢«¨ÿ?ïÿØ^qÒ>ìý/ÍЛµ>óÐÇü>>ìý/ÍЗ(4FGL J1728.4+0427¿âI>'ÉÊ+@4w%_5½À9†…˜ZÕ9À;®MnGÜ8@Øõ¥@x<¢G¾?¸á(ypÚ3?ώLßV½&@Q\þØ<@Š³áŒ?å÷$+Ž¿ãs…ô¡'¿èc¾yå¿èA~O'7Ë¿ïéÈ@K·¿ï¸ 7­ì7AGNfsrq3FGL J1728.5+0428PKS 1725+044?íh¼"­Ü?µC'c˜°?·TºZ'?µC'c˜°?ïÛï¦~†?‡U[×Ç?rz,À½ò?‡U[×Ç?êõKju?®|<Ë.´:?Ä*ÒW†+¦?®|<Ë.´<?îßj¯M€[?†d&:á*?¢	U'úS?†d&:á-4FGL J1728.5-7303?éÕ qA˜À4$ýó¶E¢À:Hä.bÀ<3+†–‡–@]îþOý@†Yùp™Æ?Ŧy{ìài?È5>eÁOì@Ü¢,æ@io‹þüJ?ïò';׿閗†™â•¿çÙ­…ߨr¿ìƒ[i³"¿ïͪB^Ia¿í³ð\ôÎAGNbcuPKS 1719-729?ï°V_Xp?Š¤ Ãõ©u?ƒûjh)äB?Š¤ Ãõ©w?ï
''ö?¬'$—@?ž­½í¡>T?¬'$—@?KA?ž2(>2&l?§ÿ"[Kîµ?ž2(>2&g?í¯ŒËߗ?™| ·O?²ƒ™¡GD?™| ·O4FGL J1728.6-7448¿å
¯£ú¡lÀ4ó*®)s—À:ÄÎG÷–À<QiQ@Ã+Ìa˜@TÔ#&v?ʧ¹"ÓÝ?Û3ÿµ­K@LÛzåy@
¢¥Em(¿âîó2'#"¿Æþž–ƒ—¿åœ¼™xâj¿írJÀm˜à¿ïÿ—?LF*?à¯:ëŽYAGNbcuMRC 1722-748?ïÛôQô-?s{¤ûTÎ?r×}éL?s{¤ûTÎ?ïÁ‡ùˆoö?¥åý²Úo?<;È&?¥åý²Úo?ë³lž[È?¯4@¹(?É2M†ß?¯4@¹(?ï·¦'öè?s'ŒT½Á|?'[BEú­?s'ŒT½Áz4FGL J1730.6+0024?Ì®ƒpg@2§Å¬À9;z6'À;¹ö&bjX@|ó€À¯³@«NoÑI?±Í .ɗ
?Âòø-}½@ìÂ
V)Ø@Ž»NöY?ï`8_¿¿ÕmÐ}†h¿â}»'!­Ð¿ã3øŠÀ¸Â¿ås•¹:¿ìEUt¦›
AGNfsrq3FGL J1730.5+0023PKS 1728+004?ïí]ôÃlI?^—ëdœ±?b¢<"¶€?^—ëdœ±–?ïöL™oS?ižõòŒ‰k?SfÍ!XÆì?ižõòŒ‰n?ïmø"©,?rf‹?'@ííŠÚs?rf?ïýZÓ¼ÿH?#®ä‹: Ç?5)bǍ?#®ä‹: 4FGL J1730.6+3805?ïþ²Å¤@?ŠDØw$ûÀ;u¬Wâ?%À<Ìè^ùŠ›@!2ÂÄá
?ü `'çα?Ôy:éàÙÊ?Ó1¹KÈË?ü7«bï¹@´=«\9½?ڊ#¥ ¶Y¿•sÂ^M­¿Åûá¸AO¿ÚÒ²˝"¿ÞødÓiI¿ïÿîͨ"ßAGNbcuNVSS J173044+380452?ïüÚ(É·û?BbÌÓ4il?9.¹²@#˜?BbÌÓ4im?ïýf+—ú?K¥ao¤Žù?4Σ@+w?K¥ao¤Žú?ï"
YÞ;è?†º…Å2®?Šü©ˆqø?†º…Å2ª?ï¡òW‹¬J?rhÑLWTÅ?‡ƒjíW?rhÑLWTÂ4FGL J1730.8+3715?ãrO™Óª˜@?WðgȗÀ:NqªgG7À<ˆ}@@úÈi»°p?þ>ΌÀmC?Á×¢é¤sè?Ç=×&ñ@R4ebZh@)ߥ¥^?îìPá
¿æèm<C}-¿ÕÞ½ÛB[o¿àÞYçþ¿âš8%
|¿ïùK ½OVAGNbll3FGL J1730.6+3711GB6 J1730+3714?ïö3æP§?Qddœ?S˜3Ñ^°_?Qddœ$?ïøَÁó?aä÷‡Ù\Ó?L™ÇÄø:?aä÷‡Ù\É?m°'O?…©«dQsQ?ˆ›d"ö,n?…©«dQsV?ïscÕ¬û?rÏ}¼#ip?'"…J|@•?rÏ}¼#im4FGL J1731.6-3002?èyÈøôž?ÿ'¶@™MCÀ8èšÆÀCRÀ:ßPÃfò}@÷–ýˆ•@HËwb?·Õ÷ÃÆhÛ?ÆCž:h0Á@
uÐfµ@¿@1{ys‹¿ïþ}êªr?ïÿùJYQ¿Ü¶ûª¿ãA¾qg¿æsßVø¿ç£5ÄÝëAGNbll3FGL J1731.8-3001NVSS J173146-300309?íª²#²Ä·?´paQfo?²ªnâiÚM?´paQfo?ÚÒÌ)žêÃ?×R5év$à?▙ë0ŠŸ?×R5év$à?é@'
"?²S¿?5É'?Êý÷×±ï›?²S¿?5É'?æcóµ"Ú8?º'ËC¹?Ó8"ÖK?º'ËCº4FGL J1731.9-2719¿£7p'ø¶@GëäÀ™À9-	¼AdNÀ:ßÀú)&@š¤Êû'@ØDŽŽoš?ÀÙÈ]ÒC.?¬øæÂR†œ?ñtŒINþk@{9ºHf?ïÿMB}þÞ¿ä/½BNF¿åA·ZtÀœ¿è,›Ÿ-WQ¿ç?B5.µö¿ÏDxjtèàAGNbcuNVSS J173149-271928?ï
û&º;0?™±Ô_ê?ž ›(¸™Ê?™±Ô_ë?ë©ÿkð/6?ÊCz°Ö(&?ÁXP?C&?ÊCz°Ö(&?ëUĚ`9B?°Åw·ã5™?¨í–ú?°Åw·ã5™?éëÖ½¹?°Úw¾t¬'?ˀP¥	ì?°Úw¾t¬4FGL J1733.0-1305?ë{åä
e³@%;À n À7†€Ǒ$À;
ì-4ì@õ ÿÿÕ@ُ¨?›dN^1ä?¿~™
,¹G@"? §?@žáW¿Á¥ˆço»¿àãÀ~౿äásLþ¶T¿ä.×N0¼¿ê:ó¼$ÞÝ¿ë.HG—nFAGNFSRQ3FGL J1733.0-1305PKS 1730-13?ïaWo¾$9?ð‡A\9¨?"Õ;xï?ð‡A\9©?ï#=ÛQÜð?¸Ñˆ<à3³?›˜D•Äb?¸Ñˆ<à3³?îÑMrPn?—Ü	`²X?¢ë(ÚþI-?—Ü	`²W?r,™?´öm;ò?Š¸ãtُ?´öm;ò4FGL J1733.4-3943¿æ§SC#Àí·ä{õÀ9cßÏpÀ;oÅYa›@­T9éç@–-¹v®³?¹œRÜpÙ²?£dûØ(¯?êúâm©Q@p
xä¿å îؐO?ãæóŸI†Ý¿èä^ÿ"Ë)¿Úâ@|q뀿æ¤0ÌP¦¿×@êÁTs AGNbcu3FGL J1733.5-39412MASS J17332704-3942172?ïÍw¿èñ?ƒ*›{'©?yD ‡tß?ƒ*›{'§?ïûÅ',Q?]
~u'ã~?@ëÃcN¹w?]
~u'ã‹?ï"=³
8?™BSÉ,Â?Ÿ/xIžY?™BSÉ,Â?ïƒã1;"?€À{NQ?8ó±ã?€À{NO4FGL J1733.4+5428?ëÐYâ@@vÿCAž0À:"Ž÷À<m‰5žG~@MTùLˆ@å!ÂÈg?ËE'Á(?Õù"›…¬þ@ I@¼?øÜWYX6?ï,B³Ù¶À¿àáô±î$5¿ìÚ _†xU¿é¨¶7_޿á"Z¿ï÷ö'õ;AGNbll3FGL J1731.9+5428SDSS J173340.31+542636.9?í´¦[†›±?¶äg";Â?²ZÍ#Ë"€?¶äg";Â?àßyT˜˜?Öp:ŅBô?ÞA
VÎÞÐ?Öp:ŅBô?é6»+ˆî€?±ÌíK]a?Ë%QÜEý?±ÌíK]a?Сæ'Ký?¸pø(ëÅ3?ç¯z¾Ú?¸pø(ëÅ44FGL J1733.6-6054¿Éʞ'ùUÀ-{¿PãGcÀ:÷8±!vÀ<0Ò­·]Ð@\U"°K@°h:{üÑ?¸ÐW›ÈH¿}Ëg<½/'?Âø4È4@+Y%¯g?B`Í ¿Û:"dKY¿äêkäT¨Ï¿âôšÜ¸o¿åLã=Qš'¿à•ªA°sAGNbcu3FGL J1733.8-6056PMN J1733-6055?ïøÙ]BI&?B
|¨Jtx?LšŠöÛip?B
|¨Jt†?ïþÙÌÈœ?@éÿ§äl/?"c3~¶C±?@éÿ§älB?ïژÿÿeE?uƒb›äÀæ?r³€M^8?uƒb›äÀæ?ïûÐC"mŽ?.®kCn<?@¾ñ®IËr?.®kCn4FGL J1734.0+0805?ïý-&·V§@4Ü^³¾#À:{÷öFCÀ;ïÁ¸œ" @*¢Ø\¢î@'¤ŠŽd?ЕGûAT?ÝûÈ£GmR@·üƏ›ê@ç‰>W©Š?ï³Ä¾
'¿áî)°•	¿è
¼`îØ:¿ë\4-n¿ïÑÙ|¸[¿íññIƒ×AGNbcuNVSS J173400+080628?í)—6"—?¾Ë˜¾±Š?¶³FK[G‹?¾Ë˜¾±‹?×ü£i€å?єwÁ¸è?ä®sK?Ž?єwÁ¸é?é)ÛÄ¿B?°†.@÷6Ô?Ë«Xíû?°†.@÷6Ô?Üh"¶ã.h?´É»Ë^9`?á˶$ŽhÍ?´É»Ë^9`4FGL J1734.3+3858?Ö¨í%g@?%á;ÛÀ8B9ҍ×À;¦ôlNô@`A–{@ÓÛÝr?òq»ÈÝC?µØçžp*@S,ü¸Lã@âà‹OÕ¿ÎAØi¿àW-^T¿äi\ð›Þî¿åÜ Ýp3¿ç½ŠÒS¿è§"ïQ0AGNfsrq3FGL J1734.3+3858B2 1732+38A?ïú|[Ù¹ý?@>ˆkO¾?F™ô?@>ˆkOÍ?ïöAçÜe¢?lcMå
û?S|0G4º,?lcMå
ÿ?ïßÝ$bƒ?uz¶"Œk'?pzmνÂ?uz¶"Œk"?ïÿF"Ý?£¸$×Öm?;¾$^"?£¸$××K4FGL J1735.4-1118?Ðàø"·Z@&p9ïôÀ:J­£;ÚÀ;Úv¾£>^@ µ[ÀE*@Cò%Kéã?ÂÍ1÷sê^?°
$àÎÑ#?ìÜ蹒]?ýiù¿Ê?âå=¿ë]ãà刅?³¹" k³¿à!ÑÁ©-5¿ä¾µÅ$b¿Ü|ö`D
vAGNbcu3FGL J1735.4-1118PMN J1735-1117?ïÃ÷½¨§?u.ãiÙ{|?~!+¬rÊ?u.ãiÙ{y?ï"E=	ZA?§ö!bž¡ˆ?‹.°½©oÃ?§ö!bž¡ˆ?ïJ'¨L?'W(φl^?–½[
ýöd?'W(φlb?í€ ¯RÆÚ?š žqh3?³þú…iÉ/?š žqh44FGL J1735.8-5932?íLRÁ(dsÀ,™¾ó'ªÀ:'çIOÕ*À<8pÇé8=@x/fŸò#@®œ£9UŒ?¿ZÝààô¿¢Ó›À\ÉQ?çGžÑÿ@a±"«É?ïòŒÝt¿éå»±–¿ê©bdy&¿Ò(>"$˜¿åuöâJ"¿Ý‡±d¼m.AGNbcuWISEA J173553.24-593204.6?ïîsýâÈz?\
 à'já?aŒ7…è?\
 à'jÞ?ïÞå®;%†?Š8éþ`ç?p(âm=¿?Š8éþ`æ?ïÌ|ÏRå·?z,­PŒ?yÁ˜V$M?z,­P~?ï·kT8H¾?l¸¿,'è?'%*ñíÐt?l¸¿,'èŽ4FGL J1736.0+2033?ïÙÂ¥°D@9kÿCAžÀ:yÇQcÀ<4¹º¡Q@`Ý•.?ûåå½^šÀ?»%33^&?Âڅ4-@	qá߃ˆ¶@L¯d‡/¿ÞTÕDj"?ïùînD˜¿Ñ0oço¿ÕÊÛ[	T¿áþàzÿzŸ¿ç#pvóÒAGNbll3FGL J1736.0+2033NVSS J173605+203301?ïý–f¸5ò?6^<¡<¦?3LÊ>Puë?6^<¡<ˆ?ïúb#±˜"?aƉŸITm?Fwq9°í?aƉŸITi?ï¿bòhoÖ?…‰î³#3?€'Ceä
N?…‰î³#/?ïëHÞì;—?S²šü{?d·!Äj'?S²šüu4FGL J1736.6+0628?ֵ՘¨Ÿú@3Ž7y…À9¢¼ƒ©mÀ;ÉÞuk¼ç@ÇÌIo4Á@ñ·?œÎ?¹gj3%?¢ähÂ-®Ü?áïk'–Fÿ@­éa'ý¿Ýê¬[¾Ñ¿å=yþHÅ¿êr(a&W¿âՌY?6w¿çiš-=Oí¿å‰á`ÈWAGNfsrq3FGL J1736.4+0634MG1 J173624+0632?ïz_̵o?'<ŸŠLÃ?´ÉR?'<ŸŠLÃ?ïìkÁî­?…Ñ7¸òêê?c"à>R!?…Ñ7¸òêé?=Zÿ?ÖÁsP?¦æ<*^ð?ÖÁsP?ï'O;<+?v¦Úö6?‹l19ðõy?v¦Úö54FGL J1736.9-3357¿ï¯¸)¿ñ];_QŸ/À9"#æÀ:cçl‹C–@'.TQ;@̧…ëfì?ÒyÜ>YØ?НkJѵj@i"a9×?ùîþ"n¿Ê±,Þ/u¹?çepûì¿à¡ÙÙû‰y¿ç.Â5D0¿ëcoÁXûD¿ïÞÜÏyOwAGNbcuTXS 1733-339?¨Ž‰'"ˆ?¨i»žª¥?îwníÙ?¨i»žª¥?ÉY;ßÝ?ÎÎ׎+P?驱<»?ÎÎ׎+P?Ð_Ø8SWÈ?´ßè÷ `@?çÐãÖT?´ßè÷ `A?­m•]#6	? ïGÑp?î)&ª-Ì ? ïGÑp4FGL J1738.0+8717?éÇ"A¢Sž@;ô`RP/À:·9©MÀ<¯b³S@cÓù¼Äí@\Óû•74?À›íܼÙæ?¢ðæ t®l?âÍ*àÔ@´@Y‡2ŽÈ…¿î®kón!?ïý­_Ÿ!ï¿ç]à…ç5.¿ÜlOIoI¿äs¦¹Ù«¿â4¥>ŠFAGNbcu3FGL J1739.0+87166C B175708+871924?ïÿ¢W}Ù?žoM¢Þy?kµDô.?žoM¢Ýí?ïþr¯MŒ?Pun
ºh?.ÈÕ'U9?Pun
ºs?ïï¿Lz ´?iG"Z« ì?`@³…ßL½?iG"Z« ð?ïÿ÷,7´>ÍÌð¦2 o>ѧ—Üá¢>ÍÌð¦2p4FGL J1738.0+0236¿¢o˜‹q¨Ä@1€*ýڋÒÀ:n@÷À;ÙYæ%cg@´Þ'›¦@ÚÁLf
 ?ÍùdÅÒ\¯?¾$jÃmR"?åü§…ëg@#+©&?éVˁ¿ØÀPýôb¿ì¥Ž¿öЁ¿íÒÅ4R$?Ð웟-WQ¿¢HtñoÄAGNbcuPKS 1735+026?îG±+2ˎ?°ã«¬—DO?«"íLÓG?°ã«¬—DN?ïçïgqF?Øòßk¦¶?hb˜Ž¹f?Øòßk¦·?ìØÀÿ-?¥=1°Ëp=?¹9ûVœ?¥=1°Ëp;?ïÛlIëÉ-?jE¬P)?rIÛ
i§?jE¬P)4FGL J1738.2+4000¿êµUgh"2@>z'ÓºþÀ;ƒšSÓ½À<7‹öBçÜ@QÎCÅQ®@©ÚßµÝ?Œ)™pÙ¿µH@Ô±s?ò¿zÊÒ!@¦%‹ªÃŽ?ïÌi?‰­¾¿êúcÿÿå¿áŽá¿Î¼¿êqH'Š¿¦I`àÚ9·¿ïþâ=ø3-AGNbcuNVSS J173807+400312?ïýmæë"?=D…Ô¢=Ö?4È§ÖõÃ?=D…Ô¢=è?ïýß$1`è?H˚v—WB?1Þtø¼?H˚v—Wi?ïÏU&¹ëž?xh¥Ö·1?xUl£
0ý?xh¥Ö·7?ïøµ$d•e?C…ñCCÔÜ?M+nmªj?C…ñCCÔà4FGL J1738.3+3228?í%êٛf@<´›ùÆ*À;8Áo¡x‹À<}uôxãA@қ&·yÔ@Ÿ¾ÿ"°?Áø¹ò8¿»ˆÖ}АQ?øÅ̒ë)¯@ì|a$ˆ ¿êÓB1Ó¸¿ä̹ìö8¿étyN w¿Í{«ÝhüC¿ïÿÿ&¦³?ïÿûÞ]BüAGNfsrqMG2 J173841+3224?ïþpG¯·ˆ?+y"0ìÝ3?(û…‡™‹?+y"0ìÝ'?ïûKû{³›?sxÚ1òOµ?BÐ1•~?sxÚ1òO±?ïÎ~3íâ?}Î"%ìA?xÀæ	Àß?}Î"%ì=?ïùú)¸?CR™³ìèó?Hß[ñ!Q?CR™³ìèá4FGL J1738.8+3822?çÌÇÞ᛺@>ȸkùÀ;îQ{‡À<ö¦€1ê@!ØÚøºº?üóìFØ
?ÔrIÞñ<™?°å#/Úä?Ù[^€=ýç?ô'=ìs±?îÝ\á0¿ïE¸põ5¢?Ö ÎAAð¿é{S]u&¿œÊîÙŌD¿Ç-q}EÐðAGNbcuNVSS J173842+382104?ïý±Ò¶è=?=dÎ&A´?2qjH¾>?=dÎ&Aÿ?ïóµÉ
W_?x-?B×1é?X"måQBª?x-?B×1æ?ï§ülÞÅ?‡&;3c½e?†äÈÝ?‡&;3c½d?Øɜ?'$GAmSj?‰–	͘øh?'$GAmSi4FGL J1738.8-3418¿îZlD‡*¿ùצ•*ŸÀ9O¡(TÀ:zòl™†N@ã""i·T@`ô¼ÕÞÄ?ÑÚ£Š´$?ѵ<O|@>EedÞ§@Õm¸?L¿æ"PA`ó`?ï%…€]˜¿é#Ê?SÒæ¿çb_I¿î'þ¢‡ÔË?©wìÎQ‡AGNbcuNVSS J173913-341749?¾nt‹ãÀ€?¾'í‹ ü¡?ì21nƒ‡ð?¾'í‹ ü¡?Ó‰Q¡CÃ?Òãíà2?æ@;W/^?Òãíà2?Ð"eÒ?³µêuêBÕ?çñ÷À6M?³µêuêBÕ?ÂåïqšO?´«ž÷Âb?ëF¿"#™m?´«ž÷Âb4FGL J1739.5+4955?²ÜæŽù+H@?·¸€®À92`8NûçÀ<CÄzî´@!;`©8@)æ~Nº?§ûîxn%Í?µ¸¡ÄË@
_`ûÃZ]@ã¤bËQM?ú+ª©¿á^Z(j'U¿ä¬…>õ!¿çêÿè­ÿ¿å•‡9᣿åE~Y¢2ÅAGNfsrq3FGL J1739.4+4955S4 1738+49?ïüú2?1ÙQ±ß‰#?8/^oGIq?1ÙQ±ß‰M?ïü
Vè?SImÉø²"??—=O€º3?SImÉø²?ï±q«!sý?;u8Øî?ƒ£•7£è?;u8Øî?ïþ
|Y?…E4<²?/.î¸:"‰?…E4<¹4FGL J1740.0+4737?×íÈ^'YŸ@?_Ãb(À:< Ÿ²¸OÀ<aë­b¤@¾éõ§Œv@$§š
\à?¼åúÆ/O?±."AS?õÔpšœÎØ@©Ì?ïÿÍ_ï©Ç¿æX}o—h¿ã1Ÿ_VQÆ¿Ùº-Ç©­¿ãQ@¾Œ¿æä&ó|AGNfsrq3FGL J1740.3+4736S4 1738+47?ïÿ>{°	v?‡Q—ŽqÔ?0‰þђ.?‡Q—Žq`?ïýµ
6YÛ?I$"0dK¡?2W–M1(Ð?I$"0dK–?ïú¸?9Qš?UGiiƒ©œ?E¹"ñ?UGiiƒ©¦?ïá}
¬?SpÄÄÃv¿?n'oòSäd?SpÄÄÃvÅ4FGL J1740.5+5211¿àÁŸ2w‰@?ÂU:Ä÷ìÀ8'Û¼SØÅÀ<#ÞËÒÒ@Eãdú@œ¦Êı?[œ"?¡ñ=;í
?ü.x?'æ@¹'ÇÅüϿϵšðg¿ãõ"!	ºê¿ç?']<9¿æm7:ÿ°¿åWZà f¨¿ê¡7¦®AGNfsrq3FGL J1740.3+52114C +51.37?ïýÐs…yÏ?+úÂÄ]Ò?1|cÔ1‰Ó?+úÂÄ]Ô?ïüƒŽ'6,?WŠ*‡ópŒ?;ãŽÆN°Z?WŠ*‡ópŽ?ïÐÓU?s.¢"?wóuU1ª?s.¢"?ïÿñ-Å
>ØÂçA]ɍ>ÝŤuììa>ØÂçA]Ù4FGL J1740.6+5346?îÙdýWÊ@?Úuy(àÊÀ:WÑù\xÀ<zp§@Xâ»Ìtb@ÀàpÀ?»Æ.£ ?½…®À>•@ÀÄù™´r@oo.ah¿áDãß»¿æ\ÄÞÁ¿âVÂïÔ8Ò¿àîÚÞÞGI¿â	w­¶‡¿êÕC^#¡ÆAGNbll3FGL J1740.4+534787GB 173932.3+534742?ïýО܋B?0ÍßãÎ*Ì?1{	¥ûƒ?0ÍßãÎ*å?ïý xÿ1o?J€öy×´¥?2ü8t"´?J€öy×´¯?ïõ}ÇÄ;´?_EM7š'?Upwˆ–>?_EM7š°?ïðéŽ?JwEç¼?^-Æãç×S?JwEçÖ4FGL J1741.1+7226¿íýNðæ§@?
¹pޏÀ;	³Ýè~À<ÂDK‰kN@:äƒøž@êp?ň.!Ña?¢¬Okx?Ü[Á|Œ˜?ùšw_²íþ?ìµæSҐ¿Ü¼ã`7"V¿æÃr ÜY¿äAß¾–ÿ¿áP2芘u¿ïÿX¥³ƒPAGNbllGB6 J1741+7224?ïäK¯5Ø?cŸƒ‡dß?k´PáÊ'ñ?cŸƒ‡då?ïƐ^×´?"‰¬‰3Û?|·Ð"v%-?"‰¬‰3Û?ï|L{_+D?ˆq°"¬á?vp"—†?ˆq°"¬ç?îÚ_ãÚmy?¯š&+?¢ZÂY(e?¯š&+4FGL J1741.2+5739¿Ø÷"vÉR@?븝jßÀ;ø¢t4À<­2.@ö睸0@eÄ÷1$?Á"ÑöØ9¿¨Í¼ì"ù?è›NÇ@
JML¹ìö¿Ø…o«‰†&¿è"Lá<P¿èbs'ƒ¨l¿à"NÿA"¿à*6¡Ó¿â÷,ò§QéAGNbllNVSS J174111+573812?ïý©Í¢–?'ì_šÕG?2·‰'ëH"?'ì_šÕq?ïýîrl?Gvby$\
?0œo­¬?Gvby$\?ïó±Yëý?X΄ófAï?XL("?X΄ófAä?ïýìÌå,?"#à‰MW?0™ŸÈ֛²?"#à‰M-4FGL J1741.5-3119?鏿å ú¿à¾+IÀ9CUÚýçøÀ:Äz³ûD¯@È©¿±V@t6¸ù±1?ËϦ›à›·?àÜ{@" @¤˜"¡¸?ü(3/­AÂ?è<ÉIŠ¿è°«#.Ù¿ÐÄ?Êñ*z¿ásÇ­©¿ìzׁ܎Œ¿îpÍÝîÞAGNbcuNVSS J174126-312329?zó¹[¹3?‡qhAöé?ïʍHœ?‡qhAöé?­OSkb~]?¾eÐD+PÅ?î+
ÉIØ?¾eÐD+PÅ?­htDô¹-?¡†YuÖÏ`?î)x»°´m?¡†YuÖÏ^?™ï­.¼?ƒJ£6Û`ó?ï0‡"–‹"?ƒJ£6Û`ó4FGL J1741.8-2537¿ç;£uÆèù@¢å€!ùOÀ8Ôê~ŽÀ:æ[{PÙ6@ &½´«î±@'ÞkZÂ?µqÞ>º$ÿ?Ûä'Z?ÜW!O Ñ@tKøÑãb?íø©)Y•ž?ëù>Dß-"¿ä΢o>¿ä8kì¸$Ÿ¿à½!Þ÷ò•¿äˆ×~×AGNbcu3FGL J1741.9-2539NVSS J174154-253743?ê‰ûwD~?ÂhµáªM?Ç¥Ø"î?ÂhµáªM?îÞ½tÈë?º'Bž¡£?¢(³~ñV?º'Bž¡£?êù"ƒ¢.ó?¶T&ÎY'ž?ÄuñwD5?¶T&ÎY'Ÿ?ì­êP?©iE´x?º¯åï'?©iE´x4FGL J1741.9+2555?ïí²Žã¦@9ý•1ã¨À;,PFipÝÀ<­^éšbí@½!ØAõï?ï0]€c½•?ø£Ðä¿?é¾ý×0ÓÝ?ût8Ùeb@-bŽÀx¿ê×ëC°Xù?ïÉxQ{¿å4µê28¿¡ý Ãô$ï¿ïÿú Âî'?ïÃk$;H«AGNbcuNVSS J174147+255443?ïÉøùeºh?"°
ØD–?{ƒM"Í ?"°
ØD–?ïÚÈsÔè
?•ôT‰?r›Æ‹ûU?•ôT‰?íwN'~@?¡p}O>Š9?´E‹ïl?¡p}O>Š7?ï—-"Çp?‰($Å}?Š4¿·N#ù?‰($Å}4FGL J1742.4-1518?Òèô
èI@פ?åÉÀ9Àºª‹YeÀ;_Œ™¦@*ò03¤r@1ú´f¤?Ðç=¼h?݆T"A'@~€8Ÿ"@¥uT ?ïÿÉ仿⸗ÁREG¿æ×í\M¿íø < ¿à— /µÐ1¿îôú¬)AGNbcuPMN J1742-1517?ì¾ðÒ?¿‡ê Aü?¿*‰o?¿‡ê Aü?àq¤7'?Ò<ÉåZ™z?ß·'ã±é?Ò<ÉåZ™z?ÝԃDß4?Àær]ßæ?á¾]õf?Àær]ßå?à-l I?»å_¡à†'?ߥ'Ê¿m?»å_¡à†'4FGL J1742.5+5944?ìFj­$]ò@?Ⱦ
í(À:(1ø .À<˜Â^§U@';‡j—ù@RI^ãL?¶WfwÆ?›šà|¾'Õ?å‰Eû7@·º×Véq?îú¨Ü,¼¿åÒÑß^¿äø!å-¿ßÈh"M×ú¿äpƒڐۿäÍÝ·×AGNbll3FGL J1742.2+5947RGB J1742+597?ïúÊñN9?>18¥´T!?DÔ:ÇÃ-?>18¥´T>?ïý6|é‡?J°[X º?4L³Â6?J°[X Á?ï÷½a.c½?X/¬
/£-?P…=£8‡ô?X/¬
/£
?ïÛe|q-?['Vþò?rMAøGiÃ?['Vþñ4FGL J1743.9-1824¿êå(ŒÓ@5JœÀ:%N1¼:®À;欇²çH@íwÜ°oŸ@Ýœ®÷Ð?Ð3rôb³?îhOt²Y"@èK èBt?÷1=ª…z(?î»ïÐð¿ç±aË×Ú¿ÔÂ܉r¡¿ëDjÞEE/¿ïÿßéà
¿êÖj€˜AAGNbcuPMN J1743-1828?y5m«ïVÃ?ƒkAö¬0?ï͕$¨!T?ƒkAö¬0Ž?'Š¬ñ•HV?Ÿ÷å΁?ïµÕL9ªß?Ÿ÷åÎ'?´'Ÿý$…\?£½BÖË ?ío¬[oT?£½BÖË ?DOØ[?2}·Ž¬Æ'?ïúì?‰é:?2}·Ž¬Æ'4FGL J1743.9+3747?î$5Ó4I@<è˜_ö"À;g5¼zo2À<»-0º²ï@g³îY?ÿuÖ[æ?çéR©ðÿ²?Ø*HþÌy@?ógÄՇ†r@œ*M[}¿ïñ4 ›–t?ïýìo¡Î¿ß¸7^»ø¿àͶ!Ãg¿ïIűO˜Å?ˆ`NQû(AGNfsrqB3 1742+378?ï⟉¶cÑ?s¬y©©?m`vIœ1e?s¬y©©?ïù'U†hã?m×7Ùîç?Kb©æ\o¥?m×7Ùîá?ítBm–?¡óx´¦(—?´_Õì"T?¡óx´¦(—?ᅵˆèC?qŒØ‡Êñ?€ÝÅøoK?qŒØ‡Êñ€4FGL J1744.0+1935?ïºÞÜ6m@7SÒǸÖÀ9rƒ\@sÀ<ÀÑìÇ>@¼ß7Þh¬?þ"à¿ÈØL?±'×
hcÂ?¢ûW¾q¯	?óÄÞ ²'/@‰Î³£?ïÿÕØå	¿ÂMæ<à[¿áìÙ|Þwð¿Õ³~G-»û¿â›õ>…÷¦¿×»s^"0AGNbll3FGL J1743.9+1934S3 1741+19?ïþ¶Ž	‡?.î~àÏ?/4—g™ž?.î~àÎÍ?ïõ2Šñ£?liû«û³?Ušëæ¶`?liû«û³?ïàǒˆ'‡?slwÚD»œ?o8mwnx¶?slwÚD»¡?ï?>óÐô'?'|
‰|M?˜!…áo®?'|
‰|N4FGL J1744.2-0353¿í5¡ä²d@*B®Ñ9CÀ9Í·'Ò$ûÀ;…}Ý{pº@ÕpK¯@meie?Öø]i?³ás¢äñÝ?î=Å}£ô@+NVÀ¿ÕpÔ^;Ÿ"¿ã
8bGõ¿è4Ž}å¿ä˜òü¿èÙïÊþ–¿ÂÒ°X¢AGNfsrq3FGL J1744.3-0353PKS 1741-03?ïá%aæW?m·Øí´¥?nڞ¨îÏ?m·Øí´ª?ïö¸#R?sÝ­ûÝ<í?Sȏ¹É\;?sÝ­ûÝ<í?ïSÈï­H¢?'ì^Æ"/?•†â
VëÊ?'ì^Æ"/?ïӕ9:,@?d=™G/L?v5cbéà!?d=™G/R4FGL J1744.4+1851?åm¿Y"@6ø/@_k À;\ŒñšÀ<™ªæÈ÷U@!v<_+߂?ü²7Pþ?ÏyïÓ»©?ªl…©?܌xžÍ5'@"`PÍ¢á?ïée߭п형";"+¿Ø¥þ—J4¿¸þ2ËYZ9¿çàm"R¿»ÉÐn
AGNbll1RXS J174420.1+185215?ïÿ¡¬o&?ϓž9¬K?"ä6yÿÔ?ϓž9¬?ïþœ*?ú?C(qÛ>ãÇ?&=^Œ_'?C(qÛ>ã×?ïõ$›Íùâ?cüh³Í.P?U¶Èd:R?cüh³Í.E?ïòy_Jí`?JÁݼ"Eâ?[
Aj%AÄ?JÁݼ"Eñ4FGL J1744.6-5713¿ätÐÉÀ,\8Ÿƒ¾fÀ:
ٖߪöÀ<L|f'ëØ@ DÁ^.´s?þњw+?¼¯éè ?±tÏ	èâ?õ­`öºÜà@xM"µm?ïÿþÞ÷¿æ´ÇóI8X¿áX(`s¤¿ÕÙjj%š¿ßWÛßm׿ää2pLAGNbllPMN J1744-5715?ïÿœ€µ!?¡þʶ?ßÒ½7'ˆ?¡þÉÂ?ïýä =-?KD4Ö|m?0Þþ—¦?KD4Ö|r?ïøM=£ý?]' F¥¹?NË	p	Ãa?]' F¥?ïøΎï ß?7KUÜ}ñ?LÅÄC|}Ý?7KUÜ}Á4FGL J1744.9-1727¿îFºÍè?6@`\÷QÜÀ8ÁD× eÀ;… Äe@ ´©‰¦²\?þú¿"íÚ?ªŒŒk‰?'Ò1n?¬F?Øvd4¾@"8­ñjf?ïò6ci\¿Ü,ûáN2¿äJ¢»Jî¿×a¿â;˜ý'gv¿Å!("-¡¤AGNbcu3FGL J1744.9-17251RXS J174459.5-172640?ïó@÷nM?Vz•õ?Y÷~#eÛ?Vz•õ?ï瞧™¹?ˆmR-=:Ò?hçaXfFZ?ˆmR-=:Ñ?ïÞ^ywê?˜Ç¡Ë!±?ž"40ÑÌ?˜Ç¡Ë!´?ï(]3™?‰IˆÁ÷'.?šÿ"MùŒº?‰IˆÁ÷'.4FGL J1745.1+4731?Ùtø½@>ƒô˜Ã°ÄÀ;T֍?ïÀ<¯l‹C•@º
.k?ýñ%Vѝí?âN.r±M?ÖÄ2I~?ù[4Ú@vkÿØgá?žÖ=
ýn«?ïÿnw¬à¿äY®'3÷S¿Ùv™ºPÉF¿é¢·…<ëC¿ïÿð ¼x—AGNbcu3FGL J1745.4+4721NVSS J174501+473247?ïõl­Ô½&?\âO`^B?U&¤V…³?\âO`^>?ïû'#|?^+':ßc?A÷ër÷?^+':ßb?ï>ƒ"þ":?'
<S÷Ä1?˜/€-x¾?'
<S÷Ä/?ïɁ½ÝD?g‹"}H)~?{w¿!]¹?g‹"}H)|4FGL J1745.4-0753?è¹Cá[Ç@%£ôË—¦À8ØûíKÈUÀ;ktà |@Ðrá@‰å\ËO?ªŠq¼
•r?†:¯1ƒ?Üùº@®@øìÂ
¦ø?îÃpbhªä?á¨Ü,¼!¿ß¢Ž4ቿâòMà]£I¿áP©ôg¿Î'ÕDÀyWAGNbll3FGL J1745.4-0754TXS 1742-078?îïýˆlþ?—eHÙ.?¡'y0U?—eHÙ.?îâÊ¥"`?»¢V°¦?¡ÓU®ýÙó?»¢V°¦?îj"$Ò|?¡½ãìô<D?®ÙVͲØ7?¡½ãìô<E?ì5¦×5Å ?«GhoÃ#?¾RÉFQ×?«GhoÃ$4FGL J1745.6+3950¿ígOڃi@=Â!yÀ:ôÿ—$tÀ<¢þ~ö€$@Ú%Oð®@ËÛjõA?ÀTUØ#Âþ¿§ñi~º?é{~h?ý‰J°Rn¿ß?ÒéF€¿æ›#Â|粿àÉÍ©kžµ¿æ[Ù_'F—¿ÔöÜÀµ½¿Øˆ]|\òÊAGNbll3FGL J1745.7+3952B2 1743+39C?ïë­a×­?`z¥iŸpÛ?d=Rž(RŽ?`z¥iŸpÚ?ïûGE2å?[îÚ?,H?Bâë»4tY?[îÚ?,B?ïÕ]2Â?xœB'?u}Qfžñ?xœB'%?ïÄÀ\¹Ø?k³*a/?}ŸÑ£ô'?k³*a/4FGL J1746.8-5235?î€
5õæÀ(v³™õßìÀ9Ågqÿ ÝÀ;ª'°H1È@^+?ô·¢@VF]²c?½—Ù%Ê ?Ï¡G"~Z#@ÔnYyîÙ@Œ>gCÜ?îÞé?Mô¿á]ʶr¿åî€F}¿æI'*K'¿î…ýÉÄÛ¿ïýß1S_AGNbcuPMN J1747-5236?ï
ÒoG§¾?˜ÈËúÌô6?žE²V?˜ÈËúÌô7?ïûR©àµQ?X²äÖm?BµX}*¾0?X²äÖh?èŽA1öÌ?­°W+¥i'?ÍÆû8'"Î?­°W+¥i"?ïòlÁò©Å?L|€ $ù?[&|¬v:?L|€ $ù4FGL J1747.1-5453¿Æ™0pþÂÀ*Àaé)#æÀ:=ÀÙyƒzÀ<	¶Å#‹ @Ä>tÎ@²ÔüF7?½g'¬lZ¿ãKX1ß?Î]èHSV@'ß–S"?ïøæ0K!g¿äFÏAò׿èèmÀÍ»¿âMrU€¿ä…áUðÍ¿éï¯OäCâAGNbcuPMN J1747-5450?ïüùÛ#0¦?3wGðuÕ?81&æzÙÇ?3wGðu°?ïÿ4e0Ùe?6Ò¾@y?sYäÓo	?6Ò¾@y{?ïãrbÄ@?o>[JäµG?l鍝;À&?o>[Jäµ2?ïüà:|†?'¤e©ÖêÇ?8ÿf,Ó©?'¤e©ÖêÑ4FGL J1747.2+4937?Уløí@>tºËB‰À;wNÍÃlÒÀ<Ø[¶	;é@!
ì‹?ý²X''†?ËsyŸSAñ? »`=ØS?Տ¤ÐÚN@Ai'^è¿ïÿþÐñ?ïÿ±üfîL¿å5=߉'æ¿Ö3)"89,¿Ùð«C"¢¿Úœå¯ºAGNbllRX J1747.0+4938?ïÿ–;f5l?žÊÈ'ß ?
q&r¥6Ê?žÊȑÞa?ïýÞ#ÌÄ¥?Iäʙ¦Áƒ?1á™ÚÍI?Iäʙ¦Ák?ïõ~[—'?U3í;ÁaE?UHÑÅ´Û?U3í;Áa
?ïúä0M¿¥?6Ã_æÐU?Do>ÉfÁ?6Ã_æЏ4FGL J1747.6-5308?ï·-s¤!À)/ñù¬ÿ¨À:oëBÙÏÀ;ö¶
¨@WS(q
^@~=½Ð°‡?Ä!_÷«¿ˆ†ê%´V?Ãì­è±î@µ›[慱¿í¸®6Ý?ï\£¥¦î¿ç{]U¹¿é6çRŠ¿ÖæÙ¾L×I¿î•¼Ê÷	·AGNbcuPMN J1747-5310?ïúÚ¨s\?OhĀuÅ?G´•^2Œ"?OhĀu¾?ïþ|Ôt?M§Ü'ÉOº?/Ž¨2¸ªµ?M§Ü'ÉO¸?îýÒìçH?˜¬ÀÊ
š? "ÞÁ1‹'?˜¬ÀÊ
œ?ï÷e¸Ë¼?F¦søvl?Q5ÀŽh…=?F¦søvl4FGL J1747.9+4704¿£µýE¦ßM@=ù'ÙýÀ;VTÊ\°À<À¿\¢˜@¯d'`—ð@é?^º z?Òu{{vn?ã–]O@	uü wnÌ?ÿ¼–ž½p?ïçÝ>´ñ¿Õ±¥^ɹó¿áÊá:B.¿é™+€À…¿áà‡_rV¿çÈQY•AGNbllB3 1746+470?ë+i_~/è?¿}п©3›?ÃRZ'@_?¿}п©3š?èÀšP?Ì¢Zϐ]?Ìÿ'—Þ¿²?Ì¢Zϐ\?åueжç_?µry«1?Õ4^'1A?µry«1?㌫•'?»³bߢ'?Øæ©òÔÛÁ?»³bߢ'4FGL J1748.0+3403¿íÌ_àè·½@;-'d2‹À9ä3|‡À<h&£Ø·½@G¨Daª@Öé5¹q?»š¦c'?»'3`)¶]?ûÿ,ëñUB@ã¸cß"¿¦¦²Ü¶¤Â¿æƒ"Ó†û1¿à«Áïùø¿ãs[ýVØT¿ë¬»Ií‰Ü¿áË¡>(¯¢AGNfsrq3FGL J1748.0+3405MG2 J174803+3403?ïírËw¨ç?`:ޞ°°?b4ˆWt?`:ޞ°®?ïýðGYË?M"ƒ¥âP??7€}Å1¨è?M"ƒ¥âP@?ïiÍ՜âP?Â˜¡ìfL?'ÆELcµ×?Â˜¡ìfJ?ïòOÊÂ%?GöCÅÝß]?[`j{ïµÐ?GöCÅÝßa4FGL J1748.1+2702¿¢‰=AyËË@9‹¬q³À:Ð	sFHºÀ<~Êl <@"êƒÁëó@­[î=`?¿ûòTEÒr¿¥QÑìqX?çÛBEõ­—@F´\"~Ϳ蝘—;ˆ¿ãƒ¤?9ü¦¿è–Òª\_|¿â'¬¸ZO¿×™ŒÃó4k¿àÓ¸^€¾×AGNbcu3FGL J1748.0+270187GB 174618.6+270457?ïýÃÿÄ?0˃Ž¼¿?7ñç8ÒÞ?0˃Ž¼¾ø?ïþâJT"°?:F1JõüX?!ÛZ¶µ
?:F1Jõü/?ïòÒHÂ3w?h²ªü–?Z[n{™6?h²ªü˜?ïür",ÎÇ?-eìŠx£t?<nÇí?-eìŠx£q4FGL J1748.5-0854?×^Þu­˜í@#O27Š°ÉÀ:…#\%šÄÀ;ݐZU¶ì@!Ÿ¦HÈF@—:*?ÃIƒ—#ȇ¿ŸŽr@†¥C?à‡ˆàcØm@^ô¶uÈY?ï"ùV˜"	¿æÐC¿dT¿ë4tF"ú¿Ó§;cƒ¾¿ãºua«ì'?Å/D%ɾ%AGNbcuNVSS J174838-085435?ïáà¬A!?r¶[kvñ?n€S¾ß0?r¶[kvñ?ïÉ0i}…?¬¤Q:Ä7?{wgËA=p?¬¤Q:Ä7?ïa°ˆMÁ[?'ÂR	µu?"ÉîöGÔ¾?'ÂR	µu?ï¸*ô(H%?r""¯JHb?õBõíö°?r""¯JHd4FGL J1748.6+7005?ïÿÏ(xG@>¶–¢nTqÀ7×m̌5À;s;BÌ-k@ðˎkß?ÿ>(	3…i?–PÕZîu?¨Œã¨±d'@'
¹t*@-…Æ}þ¿•nZ·Â¶¿ÚëèÜLòw¿áaÚ«¿ÝóÂo{¸Þ¿ãO¡ÓÏË¿âäî—!ðAGNbll3FGL J1748.6+7005S4 1749+70?ïþç@Y?»œ~0?!‹þoþ™?»œ~%?ï÷õæXét?e¡lš¨ë?P3N-¿?e¡lš¨ð?ïՌx€ÂÒ?~Ü*>©ß?u9ÿž–÷?~Ü*>©×?ïþ°Ð'y?¢žê!?$òþˆeç?¢žê!¦4FGL J1749.0-2327?×8¦ãuÝ@­¯ÑƒÀ9"¸'ú
À:©"ðÅÐY@÷i¼‡/_@KUhè!?Û¬kBïó?à›q«>Ì@GŠLáZ@ñ҆õýô?îíN·ó÷´¿à*èÁŸòú¿ëÝõéüˆ|¿îç}R;6¿Ð6'Τ=b¿âGß½•LAGNbcuNVSS J174940-232619?à9×ûŽi?Ô[`æ
R?ߌP	Ìã+?Ô[`æ
R?ÈrFº'äX?Ñ '0U?éãnQ[Fê?Ñ '0U?Ø>¡ý{'É?¾†É‡¥ÚV?ãà¯B6œ?¾†É‡¥ÚU?À(ÛçîB?»\°¶ð¤?ëõÉ|p?»\°¶ð¤4FGL J1749.0+4321?ëÜoxZ=à@=&éÝ~˸À9:ªö¹/aÀ</ë/³L@j©t@lŠ½]Ä?¨–ºÒ܏?¡§¯†ëÂ?õ꾅m@"ý™É?O?ʞΌÀmC¿â4¤ý¥Ý ¿â‰ôafL¿à"IÁj"¿ã%"R¿à–[@î\¿AGNbll3FGL J1749.1+4322B3 1747+433?ïü6kɗ?5‰Ýæ¾
>?>K"¡³Q]?5‰Ýæ¾
5?ïý]AÂÛä?N¬ê_g?5ñé Þï?N¬ê_?ïõu0Pљ?a*¸˜
=¯?UŸ^\Î|?a*¸˜
=Ë?ïé1/?U½.>›'?fÎëæÐõB?U½.>›˜4FGL J1751.5+0938¿îyvˆ[;@1¦»#WÀ7ÃãiÇC÷À;PáK	Î@ ‰ôµôï@'òeÊ?šã[üÍgõ?¹^Þ¡zRp@;'—•@F]	pl¿Ç'*t¿ÜmùÞýQ¿ãØÊfÀÿ9¿ãçހÔPпçL¢Ûa»¿èMÄC'OHAGNbll3FGL J1751.5+0939OT 081?ïñûxSÀÄ?V']B›xB?\	X~t‰?V']B›xN?ïÉ+­(–™?›\ô?{j)k´³æ?›\ô?ﵙlï?…ÍÐo·Õ¶?'™¹Ÿ¤Ä}?…ÍÐo·Õµ?ïö¤iŠk?G"˜Èé.?R·,zë*ˆ?G"˜Èé24FGL J1751.6+2921¿ÚO=(†@9†¹ÃÀ9øzYbqåÀ<÷­K'F@Ÿ6²Á@™WÚ²h?¾ólɬÜÂ?À½oø
",?þ7Ó
ÔoX@3Žk¾"?åÞ¥µ%ç¿â"Px¿è=AÞËÓ¿çþ~pHg¿ë>¥Œìâí¿ïù‡ÀÔ AGNbcuMG2 J175143+2921?ïõÈkM?Q
‹Ð/A?To)çe›?Q
‹Ð/>?ïý†ót?Mªq0Á?3Ègd[‰O?Mªq0«?ï¿Ù1¿î	?{˔–Ýh?€	³}Ì?{˔–Ýe?ïýœl^áÓ?#·*o(X¥?3ñdq?#·*o(Xš4FGL J1751.6-1750¿æ®†@''@?éúÚýÀ9¤±ÓLBÏÀ;t<"¸@ ,šä"@¦ÐNaŒã?¾&—Ÿ-¾? […â­‰¼?ål"¹™@׏SD ™¿ïƀW~A?ï÷a–5¿åZWBÖ>¿ä
º}¿ÉY¿â"ö¥
k#¿×Ïî,ëñAGNbcuNVSS J175120-175112?ï«gÒÆþ? ypüu
?œê"§ O? ypüu
?ï2u)8e?´pðl8û.?™±ZØó_Z?´pðl8û.?îFë¥'?žÉÑrNée?«˜E­‡?žÉÑrNée?î@YjÅD?™Ð̳HDÜ?«úfùS«Å?™Ð̳HDÛ4FGL J1752.1+4531¿ïëè–I¹`@=Îg×®À;%3BEÀ<†#mÃQú@Çkcü@¨> N¿?ËÀ#8?²šð €Wm?ä^¯¨Ï˜@ø&¼x{?ïþ°_-âç¿Ì7ªçݑ¿ëênió9¿Üc—¿yÓ¿ïh¿ëxá=G3AGNbcuB3 1751+455A?ï쀤ØF}?jƒ6°½¡?c['¹'?jƒ6°½œ?jzpj?¢†ˆÙYºH?Ž[¥acåA?¢†ˆÙYºH?ïi"Ö¦Ú?'$h—Ó?žòÏe+$Ç?'$h—Ò?îû_OÁbp?"öæQ? JéÙ?"öæP4FGL J1752.2-3002¿³—áb¿üøÉZQ….À9]ʊÓ-9À:""д¸Ú@f­éê*@RaœÓ
?ҋ$÷0M¦?Ô½ÝüJô?ÿ€|¬ùÈ®@LH6z?¿_&¿ë¢AsgÖ©¿ç¾BuE|¿êY`úÛ4¿ïís 3*?ïH™"º]AGNbcuNVSS J175230-300107?ë«,BL›?Æ,%d÷úÃ?ÁSOžö͖?Æ,%d÷úÃ?æò-Pfç_?Ó¹"»}4;?Ò¥_21B?Ó¹"»}4;?àç\)uw?¶Ú±…»Aa?ßÖ1G­?¶Ú±…»Aa?ÑI2àaI?¿EØW"6ä?ç[9fÏ[?¿EØW"6ä4FGL J1752.6-1010¿ÎË÷A¬Å@ K›ˆ‡"ŸÀ9Íj'E'À;rèn@P(Ð	˜@C@ˆÊ>?Îľ ¹?Ú &5j@Ž"mR?ÿ¨]—4åe¿æ½8:1
?îß®áÕG›¿áÙaÏ©¿é…V`߾¿äõ³;+¿ß«©f–7AGNbcuMRC 1749-101?Íú-|dÎ	?Åԍ¤¹øo?èt æÌ}?Åԍ¤¹øo?ڗң~ý?ÒYƒÛp¬»?â´®@õ?ÒYƒÛp¬»?Ù}8¡st?»ïäeî*?ãAc¯F{Ç?»ïäeî*?×~I'p	?¶M,Ì6?ä@Û6Çû|?¶M,Ì64FGL J1753.3-3325?Úû|«F¾À
ÐãF¶žÀ9¡Åè¬ý$À;–÷z€Ï@F³ÓÃt@uêgèG?ā¨÷…ˆ?âç@Áf<@w–¿Ê…Ë?ëX{-a¦Ó¿äBxùæá?ïøkç¿à	'Ë û"¿çM}™ù¿ïDÀ
¡©?ν{¶"¶ÞAGNbcu3FGL J1754.0-3321NVSS J175308-332637?SÐßlEeã?sð'î|a¡?ïöIÝL?sð'î|a¢?¢¸÷¸>=Ò?·GçÀ4@?îÔp"|"?·GçÀ4@?'W†a?ƒŽ˜/CŽ ?ïuG÷kÌø?ƒŽ˜/CŽ¥?B¤ªäΞ4?/Ʌµ"¹?ïûVÕFÌW?/Ʌµ"¹4FGL J1753.6-5014¿ïH¯p^$¢À(3¿ÂÀ9q¾íæøÈÀ;ÈLáZ"‹@™Ìs™@:œ£9V?·íÍ9Ú?лWYƒ)@ó ÔƖ@@Ÿ7=Xü?ïôT›bÇu¿áÔX<×ø¿æëªÞe{…¿é
áSíh¿î?S‹˜¿ïþ7=ƒï
AGNbcu3FGL J1753.5-5010PMN J1753-5015?ï~Ýg–iÓ?‹"…ˆó³ž?$S
2Ŭ?‹"…ˆó³Ÿ?ïöÍ
R!N?lÚÙîI¯?Reë[½g±?lÚÙîI¯?êјpp"?«Ã¬]ç1?Ş?Æ=­?«Ã¬]ç0?ïãH½%F?XyеÚî?l·BÚ¹å4?XyеÚî4FGL J1753.7+2847¿çþÀR@8tH@árÀ:écO͞À<SuDO»)@'°
ú> @Ü@Þ¡,?ÍÎ#äᖈ?ÁPý¢}C?ô'À®9@¾·ëêl¿ï¨"¾é_U?í4nfåè'¿æÍöÎ(Ÿ¿ÜI¹à<¿å'¶þ.o¿ïÿnªØ†>AGNfsrqB2 1751+28?ïð±Á¶€†?cöoà½éN?^œ|'þóS?cöoà½éI?ïü\¦"ò?WÉuiNÙµ?=êÎèpe?WÉuiNÙ±?ï;#o"5?"xœõ"ªÓ?˜›œ²
™?"xœõ"ªÑ?ïÞüù~P?`ÓÛöTˆÔ?pƒsÀ؆?`ÓÛöTˆÐ4FGL J1754.2+3212?Ø"ÅS!b@9hÇ\Jƒ²À8|'¿bÀ;'=mHØ·@üµ‡‹Ð?û÷BÖ>f?¤v3ãÝ4¤?ºüYxûê@'V†''@°Ž'ºR?èÄHÏ|ªv¿ÜØP÷¬¿ÖL˜_¿ÜšäN¿ääúœ>¿à#Ü~¸AGNbll3FGL J1754.1+3212RX J1754.1+3212?ïü¶;X{H?7Î5G?	?:N%<%º¶?7Î5G>ì?ïô4#où?l¢§‰Â?W͗¹ m?l¢§‰½?ï¸:L¼;ð?†R¿Pz?ñlÐñó?†R¿Pt?ïû*ºõs?1,ˆ½÷ˆ?CU*1?1,ˆ½÷t4FGL J1754.5-6425¿çwc2¦'À2yhÍJ¡À:÷È#àÀ<:©€—j@bÕ~w)W@B:73s?ºŽ4`¯Ã'?ºOM:ö?þ,—£TY@›ºø9;¿Õ6³t¿àTΎmìm¿æ²2í"ò¿æ/
¯†k¿ç¾;]e¿ä1RB˜AGNbll3FGL J1754.3-6424PMN J1754-6423?ïÞëÅ¸?rÕ¤¨Ì<?pŠ8#ÿ£?rÕ¤¨Ì;?ïðGûr"U?wXE20=?_p	×Vá?wXE20=?ï¤u¬Œô?†þ"­²¨?†â"Üúƒ?†þ"­²£?ï^˜Ë¼?}½é|=K?"-ýŒæˆ˜?}½é|=N4FGL J1754.7+3444¿æÅxtƒÄ@:
~À¨À:ÉÕTZËÀ<YT¹•¸@Q]f¸pÊ@Ð_ÿD^?Éþ¬˜ÏÅ%?Öèè÷¥¾k@×èÚI@¨þoÝ­?È+Ê^2K¿Îy™ßd©ù¿æ¬¾´ .¿ëOÀ²0¿ð?ìçìãÉWAGNbcuMG2 J175448+3442?ïì8Ésò"?k	?½^€Ï?cÇ6Œ
{?k	?½^€Í?ï÷2'£U?€
µ×@™?QšÚ¹ÝV?€
µ×@™?íE[óþ?ž†Ñ™Î¨[?³Óõ `?ž†Ñ™Î¨[?ïô €N
h?LýOë‡E|?W¾ÿcå--?LýOë‡Eœ4FGL J1756.3+5522¿ÍׂÍÞ@=¶ê šª;À:€~?¡À<e–È.›@ a®.ß<?ü6À5¯å?¶oçnŽ¨û?±3nÂUz†?ûgÿÚ$@æ~ÜÿÊÑ¿ÉîRCÙk¿ä s"6‹­¿ã€í0£?¿Á5µÙì¿ßÖ÷¿àÏ>šõ9AGNbll3FGL J1756.3+5523RX J1756.1+5522?ïþn…GÜÒ?Rãu¼?)«'2æê?Rãu»?ïüÃâ붓?LHïˆz=?9àè¢Klë?LHïˆzK?ïùrŒÀ©µ?L慻÷áJ?J5ÌýY6¨?L慻÷á,?ïê%ìÑV?Ph&@Áì?eæÚ.¨P?Ph&@Áí4FGL J1756.6+1553¿ê;"ÏL–@3PÅë1<À;ۉ(2NÀ<†@Š3Ë	@!M•¨H^@&IlÊ.?ßËƽi,"?î'­ù¢î­@ñ'À8iÔ@i@e˶Í?ïþ@Bo	¿ïü­?"¾¹?ï‹4|¿·^koe¿ääc1Ù¿æ<ÞÏ®©AGNfsrqPKS 1754+159?ïÍˁªGÕ?")|Y2üø?y?*Üû?")|Y2ü÷?êÍ<'¸³î?й`ìêÅÖ?ÄË
¹0E?й`ìêÅÖ?î
{ÒzmÙ? ;áD3žŠ?¯XBØY"i? ;áD3žŠ?ápÓbw?ÆÁõùÌ?ÝéÚY;?ÆÁõùÌ4FGL J1756.9+1531¿îÇú—ól­@2æãæÄŗÀ:ðHG—nFÀ<b.bT@»ÃZ]C¨?þ³(fP–ñ?Ôào Ê$ý?Ñ¥7<WI=?ÿZÐeށ*@lÏ,M'?ïn+÷Տ?íû.t‡'Y¿ìp2˜Á?º °º›í¿ïÿÖ_Æ	?ïú2–UA{AGNbcu3FGL J1757.1+153387GB 175437.6+153548?ïï·2`U?cB§Û@?`H͟ªr\?cB§Û@?ï;I‹?qê?µ›Êd/–$?˜–Θ§?µ›Êd/–#?î‰][`«?™FßÁ´V?§n*Iõ^?™FßÁ´U?ïAíz?"qY?L?œ7ßbP¿H?"qY?L4FGL J1757.0+7032?ì·L¦‡½@=ù…H©¼ýÀ;‹y¢ƒÀ<©ô§Ý);@!· ê±9H?ûI>‡û¤?ɳû*-P?¸4tѹ?ðK'ëk:@‰LC$—å¿ïêKÎ4«Ù¿ï']Àz"?︶•Râü¿Ø˜±ý""¿Ý/<Ùz/¿ÖAW›:ÙAGNbll3FGL J1756.9+7032MS 1757.7+7034?ïÿŶ×A>÷÷?%>ý$ý"_î>÷÷?/?ïþ/éþ)?DDÜ"9îù?-`½U ?DDÜ"9îð?ïù¯`_"?^´Œñr•?ICÆ~èº?^´Œñrw?ïø½½î«?@nŠ»³žw?M™EX?@nŠ»³žq4FGL J1758.2+6532?âi çÅìî@=ý)WÉÀ;K³ò
s÷À<¿ÇòrxÃ@ûX4õU,@åùÄ|œ?ՑBq>²?Ú*–ÁøÞN?ëáÉ^-\Ú@¬Ô=Y|É¿ìA#`Ø2¿Ó‹ûKeY ¿ä×	 åþ¢¿æjK˜"Ƥ¿éK§ž?¿Ïž¹(«õAGNbcu3FGL J1757.4+65367C 1757+6536?îêJ†5¯ñ?¡ŒªC?¡[Wœ¥ó?¡ŒªC?ïö~	"e?v§©Îþ?Sì÷ã3^?v§©Îþ?ì3Ô_Á¥Û?¦±ÍªÇ'?¾a]òÑ#?¦±ÍªÇ'€?ïµûΟHú?oöQã0ñØ?'X-Á¾?oöQã0ñÕ4FGL J1758.3+1429¿êôãaH±X@2.ä¬yÀ:'¶ªK˜…À<>­j0öB@®­€VQ›@ÍæÝð
¿?ʞÌßAC—?ÊÑJµÛČ@t¡'Œ_@dlH¨W?ïOÇão?ïþ"û¥'l¿âݸ½vB§¿ákßj‰6¿âøÀ$óª¿ïü;±îAGNbcu87GB 175603.3+143022?엦?ì?¹|SŠ§Ÿ
?»BÏö0¢?¹|SŠ§Ÿ?îMPˆËoC?¼s°8Þ?«*÷sIå?¼s°8Þ?ì'æÞ×Z¼?¬¦<¹_bÕ?¾ÀÉ	E*?¬¦<¹_bÖ?ëÜØ2r?©ÜÅÙ+øE?ÁøŒŸ7Š7?©ÜÅÙ+øD4FGL J1758.3-3028?ïÛÎÊ:À	VDÿäQÀ9‡¨ÖMÀ;$Y'¹'m@я‡G¥@,&Mq£?»J}ãÁÂ?»&@Üi"@¦¿òÉ·@λÁÎj¿Ú—"š|©?ïòZ€T#C¿âž/`?Û¸¿ä¿ó5bB¿ç(§ß, È¿áå˜îxïAGNbcuAT20G J175822-302916?ïjâ¯pÀ?œƒŽúD?'£ªþ‡û?œƒŽúD?íò‡_Fo?Óñ¦îð?³xkÅ̈?Óñ¦îð?ìqbá3?³ÇÉ:¼?¼wŸ<èöh?³ÇÉ:»?ë2³šÞùw?®|òAI?Ã51""&?®|òAI4FGL J1758.7-1621?ïm²¥GR@aXPÀ9œŒ…´àGÀ;qõ *­S@±€k^@*ˆŸvRm?Å ùIØf3?ÝÁæßóp%@ªò×ùP¹@	Ré¿KÚÊ?ïÓíözE?Éà+yUg¿æ™U ÃÄæ¿è	ÿþR€Ö¿ïÿÿ^ðP`?îÈË ÒÈåAGNbcuAT20G J175841-161703?⽑êäÌ?Оú%ö$?ڄÜ*7Òh?Оú%ö$?É?êž×¾Å?ÑîÀ…rŒf?é°XJO?ÑîÀ…rŒf?Ô¾j+«C?¶&gu—AT?å ñJê*_?¶&gu—AT?ÖþV¤~Ô*?¿Wôˆú J?ä€Ô­À•ë?¿Wôˆú J4FGL J1759.1-4822?Ô±/Å,'À'èE™gD³À9€ƒmÞ*À;úŸ[zz@Õxèt3@µJd¨ E?¸5hÀÞ­?Â5záº÷@©]'«Ž@;;-Ržˆ?ïý› Ø<¿×ÈIe#Æ.¿áñ"ý…ý0¿ä€|â©­ä¿çåöÔÞF¿ïÿö?ŒÝÉAGNbcu3FGL J1759.1-4822PMN J1758-4820?ïùz>}g?N%v¢Í×?J¶
g"?N%v¢Íç?ïüóq~œ?QXÝ3í–Ë?8dtK«?QXÝ3í–Ù?ïVŸº8X£?ŒviD!?•,¸ôë§?ŒviD?ïýŽð{·R?#£Û)!ÃY?3ˆ|"ErU?#£Û)!Ãy4FGL J1759.1-3849?áñg>ÎUÀ«Då^³À9¼~Êá:BÀ;Ñ E…EO@³WÞcM,@pöºÜà@?À×&B	?Öæa~?¶@†®â:¸@Æïp:Ћ¿Å«.1Z¿ÜR€ vÿà©
?ƒ£Ž¿à4æÇIÖ
¿ïø]߯' ¿ì#;~†BÐAGNbcu3FGL J1759.2-3848NVSS J175926-384753?ÕéB|ò<`?Ç÷DªÃ1?å^Á†áÏ?Ç÷DªÃ1?ãÔgH€µ°?Õ]X¬¡ú¦?ØW1nþ"¡?Õ]X¬¡ú¦?ÄÇWï'ñG?±LÈT|&Ô?êÎ*6®?±LÈT|&Ó?ç$‰÷ò›?°" Ï#£±?ÑÛ¶ìÈ?°" Ï#£²4FGL J1800.1+2812¿ê''a7X@6îð8⟝À:ôSËY/FÀ<›'pˆ(X@ î»J™VS?þðk®Œp?ȸLHß?"ˆfývI?Ñmâ=ž@ÎëØ֛X?ë,yÀ¶>¿ç›¸䆨¿çî°ýŽ`«¿ÚUã ÷€¿…QU)Ÿƒ
¿êG¶þ.n¨AGNbcuNVSS J180002+281050?ïþ|Õ@H
? .ÉÚa)g?(2«ûKá? .ÉÚa)8?ïþž½Qœ?GKh%¼?µ?&*îÆL÷?GKh%¼?"?ï÷"Õƒ?`:ëiB?QîöUÎû|?`:ëiB?ïù줽º?<Ë×y;?HMm	ϒ?<Ë×y4FGL J1800.1+7037?ëuBœûñ@=·hß½jYÀ:Ê,"ÜÁ7À<‰ep!@ ̀Pó8?ÿCxà¼mÚ?Ë+ëb<á?Ã;9&b?õàoP–@ôe¡o{ä?àœ)@ìt¿ã4>Kë¿â¼RÌU®ˆ¿ÝÜ›Ýk«¿êøU|3WE?´.FåA¸²AGNbllRX J1759.8+7037?ïósf§ß^??ïÅëW?Y2°AC??ïÅëWŽ?ïüþª}^?P¡gpá?8:¬—?P¡gpá?ï³57®†:?†L(¯ËP.?ƒ2²^qÏ?†L(¯ËP.?ïÏK9ߢ´?dˆêv°?xZc.¦?dˆêv±4FGL J1800.6+7828¿ï䌳W—_@=‡¤¤—À7£>d¿9À;‹Àò£öë@ò@/E@Dȍ$@?'ÃX&T?¢eÀN9H÷@(T<j@™ü)ܝO¿ÎŠ'ûG‰¿áñ<ÞC¿ãΉ/¿
l¿á؞AŸÁ¿åd]½ukè¿év"U:oAGNbll3FGL J1800.5+7827S5 1803+784?ïþD,i?(æ"éhðþ?.w+½9ˆY?(æ"éhñ9?ïùŔa6?VŸÂäªrÄ?Hé®{'ù ?VŸÂäªr¼?ïØ+ÃNï?{<£'¨¾?sêxXˆú?{<£'¨Á?ïûú·Rå?8¦ x"#"?CÜ"´oC?8¦ x"#o4FGL J1801.5+4404¿ÐQ¹1Š@;Þüz9'À8±5
þÆDÀ;ò×DÁ@~$žÅÓ^@uçÈѕ‰?¢m!à?±ž©Š@µ›"/Õ±@§¬áB¿Ñ<&âAþþ¿áÀî<‰K¿æ¡¸í÷­¿ã¡ a}ï¿ê+h{¿åQU]*AGNfsrq3FGL J1801.5+4403S4 1800+44?ïúòp¯¥?A­±ã⻋?G¬6=ApÓ?A­±ã⻤?ïüž¹–µ?P£Î¼ñ¥ö?;3JP"?P£Î¼ñ¥î?ï«ed©A?'þ´5Z]ì?…<&¦Õ¯²?'þ´5Z]ì?ïÿô«–¼p>ϝY¸…<¬>֨҇ W^>ϝY¸…@N4FGL J1801.5+2123¿ïp°óÝ@41GàiaÃÀ;½ôµÀ<Q )k3U@7œ9Üñ@ƤD‡?ĵ¤as¸¿§YÝÝÒj?å\=îx?ý3="šÙá¿¿—b¡y¦¤¿çí÷­K'¿å—ß_¡{:¿áÛ`C6¶¿ëOqºû?Ä}XEff'AGNbcu87GB 175915.8+212212?ï¼^@å5¨?wÕÞeö)?€èoƲ•á?wÕÞeö&?ï–\Åøž?¦´Åî©'?Šh΁ü£?¦´Åî©'?ïƒhG¥ï®?‰Ýî˕-2?%î"?‰Ýî˕-9?ïŽí·¼Ó?x´•òw?ŒD'øL?x´•òx4FGL J1802.6-3940?ê•R$gŽÀ ×d­ÿ',À7†Ã!À;/kn
#Õ@÷ZšUVI@ºÞ¿q?›0œ]¡ÏQ?Àƒä%®æ2@!+ˆ‡"ž@ –žèc¿´õ¶6ˆR¿Þž K¿åH'NI9¿å±Wü@X¿éLõ‰¾¿ì¼Ý5МeAGNfsrq3FGL J1802.6-3940PMN J1802-3940?ï"d.%t?…?eoß^â?‹&úôv¢ú?…?eoß^å?ïÕ"#=,?–|L¦6œ?unîazj?–|L¦6œŽ?ïM'…jÍ?'Á\ƒ+,Ì?–M¯_r¦q?'Á\ƒ+,Í?ïü¹ªrw¾?2ŒDX:BÄ?:2¬lB´?2ŒDX:Bµ4FGL J1803.4-6510¿Þ %™ÍˆÂÀ3¤çÝÊKÀ:Hð3Ú"À<')H>@åWáY@;hê?ÀyYÑÇÞ?ÁÝÀåãÊ@Y%5C¯@»ž;¿É¯?Ð$¿½o·ž¿àt•žbV6¿æ~|§ñK1¿é\VbbJοâonLå¿ïÿú@ùDzAGNfsrqPKS 1758-651?ï÷ª²ñjœ?N,¸nlæ?Pªš*Ë0?N,¸nlåè?ïüÒè<ˆ?U

$>U??	h¾²€?U

$>_?ï£Â¨j-?'}fw¸ç˜?‡UåtºP?'}fw¸ç–?ïÖ½bÀ¸k?_–š)2-ï?t¡NŸ£Ê‰?_–š)2-î4FGL J1806.2+6143¿ï–O£½Ý@<ô¡7óŒTÀ:­FBÐ_À<ˆ¢üïªG@Y€Œ­M@ÒÆü©3k?Èg¨Z҉z?ÉqBãTy?õÏíé}¼@ßÿ/ögÑ?âXO'RÑ¿å9ž»'¿êi8"†<Æ¿êpBóš–ð¿î¼üJÈü¿ïÿø¨ó©°AGNbcuTXS 1805+616?ïûÚ¡‰Ð?CfxJÃ?@•{ØÀ¦?CfxJÅ?ïôä="èä?rԔ­1€÷?V7"Ö.4ß?rԔ­1€ú?ï°ÁÞFži?bõþƒ?ƒÏˆnXe¶?bõþt?ïš%%1ö0?w³
(8¶?‰v¶³'tW?w³
(8¶4FGL J1806.3+5345?ï~a½X"2@<²[1~þÀ:‡Ç™kvÀ<oaÊsc@³IÁ?%@¸;Ÿé?À×Î.äð?²Î¤¾:ã¬?íü¿øÓç@y³Ž¸?!¿æÿ'æFñV¿Øò­œ…Ý$¿æf~ºC¿éQæýz"œ¿ãI‰›á¿åݖ^%ÐAGNbcu3FGL J1806.8+5346TXS 1805+537?ïþœ»½,?-F;Hۋ?&4D-@™?-F;Hۊþ?ïþCC¸?GŽmRF¿U?/ËϻĐ6?GŽmRF¿a?ïÂ6ÕÔ§?|à~Xf?~ä•x¬€?|à~Xf?ïø2¾2×?;ÛcáQ"l?O5ù4¤±?;ÛcáQ"74FGL J1806.8+6949?탑qBx@=*½¨!óÀ8
|à%oÀ; ë)¯%ó@®MÈ_Ö@ñuù`¾?—òu"§¬?ª%û÷:@®›aöK@ÄÃb벖?ïý6Â3엿àùÛ=¨×û¿äõÔ-^'¿ãe.Í/ô¿æ].yÖ¿êo¸õs~AGNbll3FGL J1806.7+69493C 371?ïüï´´â?;[z!ß?8‡
ZXïÕ?;[z!û?ïÞڌ·w‡?öW–jƒ?p'¹¤D<]?öW–j"?ïÇ_œšW¾?ê‡Jż?|P1²Ô ?ê‡JÅÀ?ït¾ß¡ÿÌ?|cÕ!6?'h$À?|cÕ!14FGL J1806.9-8038?݀IÕÆhÀ8öt)ˆ<À;Vm¾iÀ<±>K•)È@ á'&³ý?üþ¾œˆac?Ñcz"ÛÍ?ÆqLN÷?õ,JŸ`ƒ@ƒ»ùë¾Õ¿éÓÂõ³uä¿ïÿ½ 	c?ïü•¢i!¿Ï虚eG¿ìTտ到?ÐÑ"D¿AGNbcuPKS 1757-807?ï÷sVʁC?Ll£¨T5¢?QRjýz?Ll£¨T5¢?ïüƒØ Ýê?W#j9;?;á:ù³s?W#j9;?ïXDڞë˜?Žsž×dÿK?"÷d¬" ?Žsž×dÿG?ïÔìfqý?k'ýL·ç?u‰ÌÇ8Ã?k'ýL·å4FGL J1807.2+6429?ïMb ¸NÊ@=Gb• ŽÀ:øã`'À<רª˜@ !
]¦ú*@¿»lR9?¿
…&}˜¿ŽöjÍJÃj?юÖ<b0ø@	¼‡°8?¨šák.¿ÛJÿ"	•*¿â»uÝök¿Ó[<'¦¿å0¯?ž%š¿ã}|BםAGNbll3FGL J1807.8+64277C 1807+6428?ïÿ5¸ºl?ª"ì) €?H轒"p?ª"ì) e?ïþJ¿TLÁ?E[-B\?+T
»3÷"?E[-Ba?ïùø¬ql:?^jY8'ãR?HN:O'?^jY8'ãK?ïþWm{(Œ?{°zÄ&?*‰(MwZœ?{°zÅi4FGL J1807.9-6412¿ïðбRÖÀ3ºnCªy¼À:Mð÷3©À<Ò¡"$@b,™!O@Lë]±‹ÿ?¿bVz]?³,Û§?òö`ÿõE@ÿ@±K ?ïÍ>¬ãù9¿âĬ½bÌ~¿éñ9ÉOiË¿ãRžÓ•=ê¿èó2ýƒMþ¿ïÿôÕ÷AGNfsrqPMN J1807-6413?ïüGë?B •p}˜?=ÇŸ ­¼?B •p}™?ïü+Fؽü?hLp`I9A?>¥É:?hLp`I9B?ïr"C¤?}"ªÚø2d?~¹FµÞ-"?}"ªÚø2`?ïꗒ/î?R'9šãä?ehmÐôæ?R'9šãäŠ4FGL J1807.9+4650?Ù·Ž_Ÿ'Ò@:'ú'è},À;*ƒì‰*·À<Êˀœs@ 궦oÀØ?þW§6:N°?ÃÁˆ5™¿^…'Wîå?–V»ÅàÁÄ@K\YQ?ïrÿ0Í'f¿æþíþ¿Úw
"˜±<¿ÞÒÕºÝ3¿ÞJžß©žJ¿¶ìKÿC'ÙAGNbll3FGL J1808.0+4652RGB J1808+468?ïýp%Š5û?-Á'ƒÊ{?4~Ó®P."?-Á'ƒÊ7?ïþ°øTõ"?@ôN>Ñ]v?$ðz°¦·ô?@ôN>Ñ]f?ïø®zËB?VSÄî£H?MFӂø_?VSÄî£C?ïóV­×ƒ?E6ì´!Ù?YR¤Pøýn?E6ì´!ô4FGL J1808.1-5013¿äFp6Ü£‰À,.ŠqÞi­À:Öé†@÷À;ûŠŸb0@fÀ'¢Ü@‰ÉºÉ•
?¾r]?¡+?¢I=`³žþ?á±+6½+@MΛE–¿èÙÞÃð/¿Ù…=jĚ¿é§1½gT"¿çÉóïT6¿ÙÙÁY|¿ïþµ}$îÍAGNfsrq3FGL J1807.8-5011PMN J1808-5011?ïý*é¹ò.?6½àçûj»?6¨²0nÈ?6½àçûjÜ?ïþÇ¢$ø^?=.\w	þ4?#…Ý°z;?=.\w	þ??ïžEˆ2¾?ƒÝŠóªèz?ˆnº]óOî?ƒÝŠóªè{?ïü½Œ¬ž6?.C;ŠVç?:š›N»?.C;ŠW4FGL J1808.2+3500?×Ëãî2ßx@7uø>ŸÀ:&ÀMb‰bÀ<=JYPÔ@,'úÅÙi@ÿ:Þ"_¦?»7ðÝ"Zs?°_y[X?ó;ëh™@	âæk"?ÄZ÷ÝǛà¿äIÜݼY¿ä&»‹[é5¿áHí¯›d¿ëª¥Gá@?—Ÿ÷y7AGNbllMG2 J180813+3501?ïï±´t?SOڊà`?`àêNK‹á?SOڊàY?ïýp¯ö	?M´¦Ñžñ?4z‡ÈO·?M´¦Ñžä?ï¢7Ýg?ŠKMK"ß?‡|ò;Ȧ?ŠKMK"â?ïá"^Ÿ÷Ñ?Y"à6+'a?nÝ¡`.r?Y"à6+'`4FGL J1808.8+2419?êh	Y\è
@3¼c¾ì9zÀ:Ïì""9À<XÕï‹=¶@ D›—ËŽ3@ð+[Î\ð?"J_Ÿ¢È?(BŒ;À?œ¼bØxÂ@1øûÔÍ!?ᅥ",˜¿ë…ë1;â.¿ÙÍî \+z¿è/V•8¿Ä FÜÞ<â¿Ý‰/žÔAGNbcu1RXS J180847.3+241923?ïúw}y'\?B§¿Ôä?F"
º')?B§¿Ôä?ïþdkÓìž?ITëgt!?)¹BÁ6ÿ?ITëgt.?ïæà—a@¬?q|"è¸á?ihž¿SÀ?q|"è¸á
?ïøØêÇ?@,oy8×Ï?O—ÌœTބ?@,oy8×Ò4FGL J1808.8+3522?çªÛ>šB@7s²$ªÚ4À:ß\×qk}À<u¯§"Y@³ò ™R¢@EĚÏ#¿?щĄ©Èf?ÚPÓ!z¤@w|7‰?òI"Ž³°¿Àgّ×-?Ѩ¡ÿïŽï¿àx^졬¿à²öañŒ ¿è»ã?ÕÙ¿ïøbý¦3†AGNbll3FGL J1809.0+35172MASX J18084968+3520426?ê¤kÎç¨l?½—‹3¿¿?ÅnPÄa^M?½—‹3¿¿?×B"PïP?ԏ'ðR*Ñ?ä^î×ýW?ԏ'ðR*Ñ?êg±"®Bj?«óéO)?Æa9íFöW?«óéO)?ÂQb"±8?¡jù×?ëk§wxS²?¡jù×4FGL J1809.3+2042¿ï˜ëcýe@2Ao!öÊÍÀ:>Ï#¿!éÀ<VÇM1;@†Ò£¦bÖ@§—£öî?º£ÅA"¿w8uKï?¾]‹¡^_@Q
9òÑ?ï\6f¿½{B*8¿àŠUú˜{¿ã®bHŸ¿Ömt¢"?¿âG àö$ŠAGNbll3FGL J1809.4+2040RX J1809.3+2041?ïË˒õ^?p*Ð=e
{?z6ñ…P?p*Ð=e
|?ïü?ȋù¶?TäXµ–?>» 2OÐ?TäXµ¨?ï´à_LŽd?'ÁŠÎ‡#õ?'Çè,Üg8?'ÁŠÎ‡#÷?ïÈÔР¤p?j<Ìx´EÂ?{•—¯­ÇÖ?j<Ìx´EÂ4FGL J1809.7+2910?æñ·ëÀ^@5EV:Ÿ8?À9ƒ-±éòxÀ;í.I¼â@ꊁù"×?ü3=D.-:?µ'‹>s>w?¹Æ]qö•@Xå>³™ö@YmÇXÅ?ïàCß銿å×Ù`.¿ÓcY%¯g¿×#¡šÄçÑ¿áa'·'I¿á€0q·ÓAAGNbll3FGL J1809.7+2909MG2 J180948+2910?ïýõjãŒÿ?*ûàøoÜ?0T¨ã˜Ù?*ûàøp?ïðíVzX:?zïÀâ3?^%SOŒ•?zïÀâ6?ïÜ1Âz8ß?tpÕÇÁi¿?qçÂã'@?tpÕÇÁiÁ?ïÆË]\–%?bÄÛü""?|šQQ´í1?bÄÛü"'4FGL J1810.7+5335?ï×l™‰ö@;i_JsÀ:[Þây|À<'d}Xs@¸ŸJ;?þ¸\'·ÕÅ?ÂÜýŸ?º>—ãåî?ùž˜5@ "ô>?ëf?úìÆ¿æ‹vÁ¿ã±MëE]Ø¿Ñ¥øã?ì¿ãÃ?»òn¿áAÝ¥¸AGNbll3FGL J1810.7+53352MASS J18103800+5335016?ïøÉš!?F|M	U?Lۃí—vƒ?F|M	^?ïí³$‰œö?z—€
§%?bLÛvc	´?z—€
§%?ïãsí"k/?w,8R${Á?lŒݔҫ?w,8R${Á?ïppì?¬«*þ][?œ1ðñâ[?¬«*þ][4FGL J1811.0+1608?åËóWÃj@0ٜ¾èÀ:UáE)Õ¼À<7tm&S@ •R&é?ÿaýKÙÆ?ÄTPåÔÝ?À¾õHÁå¾?üŠ=Ü¡@
ÐÏ֗{Ý?é?÷!	:¿ékÞuk¼ç¿Ý¡ ñ§£¿ÐúBœÜ=¿çÎ8§ç:6¿å´ ÓʘAGNbll3FGL J1810.8+160987GB 180835.5+160714?ïû{ÒôC1?@j}ìž-h?B´.ó:Õ?@j}ìž-i?ïü‹Käa?WøÊ-ÍÆ?;¥ ß])?WøÊ-ÍÈ?ïê(áãç?nXÀ;…ý«?e×<Xy?nXÀ;…ýŸ?ïôèGíð?B.ëÃö±š?V/p%Ü!«?B.ëÃö±¨4FGL J1811.2-2759¿ìT˜Ý¿XkÀ£D^Ô¡­À9ðb¿¤À;¦Ù>Ëê@ r%|ç1R@
òœj.r?ÁÅ[¿Cw?£P»¯C$?æòûE•‹@–šÆÀCR?ïI¤^ïz¿å¸ýÿÚ¿åìŸÀÐU¿Òõ¦n"2¿ä›…AÚ¿Û``="(AGNbcuNVSS J181120-275946?ïðÎη´?[6S"å ˜?^cÞb"é?[6S"å ?ïýQÛ
™¼?V'ØïB?5q'«2ƒ?V'ØïB?ïžËuèJ.?ˆVØÍZÓû?ˆM"…ítt?ˆVØÍZÔ?ï¬æ•þ?qEªoçG©?"ûF`€º?qEªoçG§4FGL J1811.3+0340?ï3ªXX<Í@%4¢v·íBÀ9-Ôx'¸ÕÀ;®n@O{h@ßqÎ#Žû?û±ëºÎ‡?±zƒ(éÙ"?¹£Íúõ)7@2‰¥/ÏÑ@ ý+¿ïÿýFKê?ïÿàU?Íu¿Ô¼Q?Û0¿×a!§¼r¿ß
®ñð¿Ýî–áƒh*AGNbll3FGL J1811.2+0340NVSS J181118+034113?ïÿ3?@S»?WOtŒªü?˜õˆŸg?WOtŒ«L?ïélHšh(?}[H²??f"·e—ØD?}[H²>?%ëi\?'ú
0È P?€Þ…%¾¨ã?'ú
0È N?ï´_3ôø?rí°ùšîê?'ú(3ÁÝ?rí°ùšîí4FGL J1812.9+4249?àyàN2ð@8ÅAt>–>À:–´ -œñÀ<g&••þÚ@¶-÷ `@s¤<ŠÊÊ?Âù©d<ën?£ªËñº?ß)í9SÞ¤@q‰¢¬=?ŒUe­È"¿çÏ d#–¿ç(9À.e¿çê	*v¿äµ`iÍ#4¿ïÿäâBTäAGNbcuNVSS J181308+424853?ïö™ùS'?R{ç›V?RÌ
Yû±|?R{ç›d?ïü¡ieNQ?ZsÌJo?:ô´Õ†~?ZsÌJs?ïÌ.é¯	y?yÔßÆO4?yè‹({C´?yÔßÆO6?ïÜZ©X®?]FÒffã|?qÒ«xS¨ñ?]FÒffã|4FGL J1813.5+3144¿àø¶áŸq@5`RÚšÀ93®üm¾À;Êù²Þäý@çƒzú@E"FK=ì?¯‰ðÚB[?¢èׁÜ9?ôÌF嗞î@
KH¨»J™?ïñè°X"¿åT}e†l–¿Ýs>#§$¿äloàŋ¿à—¦°'«¿åbf'P¢AGNbll3FGL J1813.6+3143B2 1811+31?ï÷Þœ?KÞz¯Xøf?QÚCÒÇý©?KÞz¯Xø_?ïûÀocN?U.ëñrz?@þCÞrÈI?U.ëñrz˜?ïЗD¹m?yd˜PV5L?w´]£IrX?yd˜PV5R?ïáL›hµ,?Z^÷<JIÌ?n³d—JÕ?Z^÷<JIÇ4FGL J1813.6+0614¿î[bIˆÃÄ@&xžÛø¹»À9…È•/§À;Û$
¡C²@kىô‹?ýñ ¦ÔÀ?¶•ÄÞýã?ÅyÞonM@¡ÃA2Ð7@	H€ô1?¾¿·ë˜iî±#?ƘŠ:N¿Ô>ðÁ¿ݏO(\?œ¿ä}Ëùï¿çK`6÷cAGNbll3FGL J1813.6+0614TXS 1811+062?ïˆúlƹ?"8^ˋ«K?ÁdÎQºý?"8^ˋ«L?ïµHøÀ?–£@¤msy?'­ø»ϓ?–£@¤msy?í<_*§˜?¦xW.˜÷?³ªÃ>?¦xW.˜ö?í×2îÈ̬?k3û?±Fh‰¹š£?k3û4FGL J1814.0+3828¿î•˜@7dÝDUÀ;l$ˆþÀ<¤$u*Nˆ@Ùܪ»U@!€[2•?Ãé•Zo¸?€ËŠ#ý,³?ÁQ׎â@…DM÷?ï˗C¿äª¶ÂŸLa¿èo,s%'Š¿×j,#tyO¿Þž^då1ó¿ë/…>BÛÈAGNbll2MASS J18140339+3828107?ïüú:YÂ?47>Óvµý?8/&-1òU?47>Óvµù?ïþ¼*âÐ?>ýÖTŸ1	?$=Qßõ*?>ýÖTŸ1$?ïïÐM¿Y1?p#(®ú?`/²@¦Ïu?p#(®ý?ïùÖ¤î?82,^)¾¬?H¦lGº?82,^)¾¬4FGL J1814.2+4114?ê£C{}j@8 9GIj­À;²_c<æÀ<…"f+®@ßÁ_±@@h–<"?ÍøU¼ ì?¿ó¬-AØ?ð+uϏö@Wâko°?îQ6ßD—¿ÝÔäžO¶Í¿è08­¿è´" [Tº¿ä2ÙaÒ£¿ïÿð`OËðAGNfsrqB3 1812+412?ïü"Ì7Â?="ˆj5l£?>ï!žAðð?="ˆj5l‹?ïüp†@\?RŒ<¹¤Æì??Ü{Íýî?RŒ<¹¤Æè?￧ë(ü?|qÐ}Ô??€5Àý\?|qÐ}Ô6?ïÕ0ÿ™¥	?^ËQÖ'?ug€3-{Ð?^ËQ֐4FGL J1814.4+2953?î?—Ïvý@4¹à`þHÀ:œÁr%·À<1ýKÙÆ@¹‹cÅ@EI@»²?Ņa(c÷K?³ÄÓÚGó?ìö®G¦‡¿@
è§á6¼¿èIžŽ‹t¿á< B¿çÄä þé¿æô,Ý®œ`¿äª$+X¿ïÿ6a;aAGNfsrqB2 1811+29?ïþLH:ã5?-`gºQB~?+;|Q̶B?-`gºQA»?ïý}W ËÏ?Q]@hÍù?4Fù¡ˆš?Q]@hÍù?ïØ*'ûì?u&L÷ÕL?sêø¶'.?u&L÷ÕL?ïøð5Ís†?<PÓ·À?L?(Ê1ã?<PÓ·¦4FGL J1815.2-2715¿‡¤šZ;"À_óÂîÀ9f}å,õÀ;7sx @=ϕÿÜ@®ï¼»Ý'?Ã_À‡'?Äÿ{á!îg@±ÕÝ톁@~žHªé£?ـR`J¦?íØRÂD³Ž¿åþ‹÷§q¿âÊ¡yaë­¿ç&r@T"¿ìÔ(᠙hAGNbcuNVSS J181510-271304?ÝéIÊ
ž×?Ëýp‹Ýjç?á[ú°•?Ëýp‹Ýjç?Ü´øO£+?ÕG4Øû±Ö?áø¥ƒØ.j?ÕG4Øû±Ö?ädØÌ8_?¸&ýô?×6NgÁA?¸&ýó?Ñs!XQï?·LÏÍ¡p?çF~oS×?·LÏÍ¡p4FGL J1816.9-4942?ÙZ㯈ŽÕÀ.U¾'bEÀ9¡ÑÒÆÀ;ðH±I¹‡@mÇ՗ Ã@ôÉBԐæ?¶Í¬½?Æ®÷ϯÖ@Ðì1"@\ÁÂ,µÁ?ïøè^£¤_¿ã´¼j~ùÛ¿âqÚ}ºjõ¿çƒüÿšs¿éâ@!-L>¿äÔê"H)dAGNfsrq3FGL J1816.9-4944PMN J1816-4943?ïÐEPf®{?ykpt£_?wÝW̨Á®?ykpt£Z?ïú=ǹ€{?\wNô}^?GáþÀ?\wNô}N?íŽ5"žÂ?¤Ã¾œ¨ÖŒ?³6S[	ë?¤Ã¾œ¨Ö‹?ïîõ''Ë?J}e²‰?að
Ø}4R?J}e²—4FGL J1818.6+0903?înt´4Æb@&¸÷QÕÀ9S€éŸkkÀ;¨J¶Ýw@÷—´&¹@#z›§Ó?µ8ð6‰T?ò	½n
@
Jè[žŒ@(2Oˆ~i?ÔÒ«3=¿ÜºÂÇ;=¿å?çÁŲ§¿å{C؜䨿èeçPÑÑ¿ïÿ5Õ¤â£AGNfsrq3FGL J1818.6+0903MG1 J181841+0903?ïÝÔØæk"?iú¯'Û`ù?q"ŒÊn÷?iú¯'Ûa?ïó;ÆÖ}ù?r¸¥°×0?YˆrS–?r¸¥°×0?îÒ<Ÿ,O?–••Ûu˜?¢Ü6
7ë?–••Ûu˜?ïòTÇ?F>ٓ>5?[ÅWÌq׸?F>ٓ>,4FGL J1819.1+2133?ÚM\ùÛ_$@0~ýX…ÓÀ:P-zŒŽÀ<L|tÅ¥@í	Yp	@tw·?ÀɤyF'á?ŒkÕÄ ¶ø?ϵwß?øüyzë-¶?òÉâ¿è,YÅn3º¿çe`¬é¿ÊU?øh†ý¿Úð®=ës¿ê¨U¿O5ÈAGNbll3FGL J1819.1+2134MG2 J181902+2132?ïïó¯Nâ?Y'²Î&—?`þP±´?Y'²Î&•?ï×ýîÙ?‡®Ú
"é?t"póÛ?‡®Ú
"é?ïÜ);2g?w–ЦÊ	?qëbfóL
?w–ЦÊ	?ï1Ó=æ'?hýpü}"?™Å˜C?;?hýpü}•4FGL J1820.3+3624?ÞÖRèj-E@5Þzt:À:"Y~À<ƒÎod;ê@ èíˇ'?ü5ˆ]13?ÂêÄ.˜š?§%E<}½N?轶ÿÛíÒ@½rã¢QN?ïêÒa6PÊ¿éV!IÑ°¿áãп "`¿Ê"~èx~¿ÑÐrß­*¿ßlg1gAGNbll3FGL J1820.3+3625NVSS J182021+362343?ïþ?Â?$\Öh0¦]?.hÎ+?$\Öh0¦%?ïý"«
íÙ?PƵw=¡?3Z§'?o?PƵw=™?ïö­Æ¯§Ô?bÒ:™ÿ2?R¤r °Y×?bÒ:™ÿ4?ïîÙZc?KFޏ?a&¥rœê?KFޛ4FGL J1821.6+6819¿Ýâ]xy•@;Ìú¬Ùè>À9<f0¶1À<"øR@{ó&þœ~@—AЄè?«'ÈûîÃ?ªâðz¦å?÷ÀW xF@9Ê&)?ª
‹ýáB¿çö!ãÕ}¿çÛÓ/½\í¿ècúÿæ¿ëÑT†jí¿ïó'^±ŽAGNbcu7C 1822+6816?ïþ5\ª?%µé	¦?/ì®:5]?%µé	ð?ïýz§3Ž?J#¼e«?3"*Æc˜K?J#¼e¶?ïÞtP±Ö0?qe("wWã?pÅקè"?qe("wWå?ïýr;æc?+‰"9.'I?7Ôn Ìç¨?+‰"9.'|4FGL J1822.0+1600?ïz'\¼À@+0Ãóà7
À9úmû†¼À;ä$>úè@‹hÓ©@2¼›&b?ßàŽ¾?ÁjýyèÏ7?ø¥=§*{Õ@(",J
æ¿É]q¾‰¿æ@³^'°Â¿åJ*Æ}'s¿ìÿGþò8í¿ÑfKÄ#°ß¿ïï©:÷LÓAGNbcuOU 134?ï¢ÅJÛi´?"o½l9›ƒ?‡N­I%"?"o½l9›ƒ?ïڝczk?‰ò}9Ÿ;?r±ÎBʕ?‰ò}9Ÿ;?îd¿W,£Ö? µK
k'q?©´
5? µK
k'q?ï›Ê܉"?wµé§|cæ?‰8ÍHݟ	?wµé§|cã4FGL J1823.3-3720¿Â««LDhŸÀ%íîÇÉXÀ:Î/OxäÀ<‹Fí$[)@@nå»Ü@Ô@C¼î2?Ôæ|+õ|?ïÿø]Ê5™@Ç%Þ¶Ú@›ëƒq9(?ïà7]d_%?èïÕ¿èÀc'†W¿ïþ.~Ãq?ïYِ)®O¿ï¦€g™lMAGNbcuPMN J1823-3724?ꬶ"F?ɯŒÇ~dã?ÅOŠ%îë?ɯŒÇ~dâ?ç±ô39Pë?ÕÝAû¥Ç$?М™^+?ÕÝAû¥Ç$?ÝÏ5g&°?ºðæ#)õ?áeLpl¨?ºðæ#)ö?èOéøø?Ê=¦Ç`)†?ÏòÀYø?Ê=¦Ç`)†4FGL J1823.5+6858?Ð	`'Þä#@;«h¾/{À:(ðzPþöÀ<oE§©ý•@vb)?êQ?ÿ…C5ßµÞ?¹Ãy'çI?Ðît1Žî@«>o§X?ûê"Ò/¿ï@)æÙ?ݤQ¦ùT¿àþ3ÂOEc¿Þæþ¼³úï¿ëüYýÍJÌ¿ïÿùµc#¼AGNbll3FGL J1823.4+68577C 1823+6856?¤Wó§åµ?¤˜`‹ÑÇ?ň¦?¤˜`‹ÑÇ?°,p¯º{?¾¶x½n?íúqê½1?¾¶x½n?²%`Š)é?¢Ï:\S?í»Sý®ºÄ?¢Ï:\T?¼<e9—?¢Ý€åTœ=?ìxs\nÍ?¢Ý€åTœ=4FGL J1823.6-3453?ëwéÜZC®À#ß6ï€UüÀ8¦}¢ÃÀ;~ð=ë@ça•q@à?û(œ6,ø?§}–¦B¹?«ß¤jØæá@+Còž@û´^kñ?ç$çá¦?ïù—02ͳ¿Ö[œ¾'!€¿ÒŽ"&±¿à_ZοԪÂ@ÆAGNbcu3FGL J1823.6-3453NVSS J182338-345412?ïüÚUUf?8ó*í2?<-UTʇ?8ó*í2?ïê:Ï¢"®?‹ëä‡ñ?eÅ0]lQI?‹ëä‡ð?ïrÎA§?F^'wñþ?'¦7Ýkð?F^'wñþ?ïšêþ#ôF?{0ó*·C?‰E@wî¬?{0ó*·Bÿ4FGL J1824.1+5651¿ã<ߘTfÝ@:Ù#d»À8w–Б}kÀ;ÛLg"t@½vá³¹«@o	R
?žöÐ"äþ¿?°'²o~h@§Ó[\G)@k#Bû'S?Ë%=|7^¿ãT"Ö¿å¿ž ß¿åÚÛo›ï¿ç!ueݪk¿å#slß&lAGNbll3FGL J1824.2+56494C +56.27?ïü¦Ë…ÎZ?2ÄVëª:ß?:ɣэ()?2ÄVëª:Ð?ïùÅ[cþè?]"vô#â?Hê'pa?]"vô#ã?ïÕ0l¨*ó?u7MYµ§?ugÉ«ê†Î?u7MYµ£?ïø€îÕ@?>ɓå£"?MÿøD«j?>ɓå£Î4FGL J1824.5+0107?ëìâvBÙ@ÃX¯Ä~À8äB(™|=À;	‰H¾I@.<<œ=Ž@.—eóS?¸Ôž}Y&?²+
Ò&?ô~žš@*êëñ«)?ê¯+ie¿åù	p¿ëgV@S'3¿âT	×ð~¿ë^*Ã") ¿ß&a"˜ÏAGNbcuPMN J1824+0104?ï"	"÷o+?Šk-ÿ.x`?‹=›$5?Šk-ÿ.x`?ïór%dÖ?oÝōÈX3?Yµ7ÌUw?oÝōÈX8?î1y°A?žø/xŒÚ?¬î(d÷+ï?žø/xŒ×?ﮘ-ÜèÎ?p!·©W?"YôˆÅÌÁ?p!·©T4FGL J1824.5+4311¿Üý³1e· @6ׅ@FA-À:Ô{bvíÀ<+¼FlÌ@!4Ö½;ŠE?ûÇ(-E³h?ÇWOGß=?´àú@ÎQ\?ð܆Ô@Í:Ó»~q¿è¿!Í°"¿¢I÷<Ynÿ¿æò•^KË¿ß!š•m¿É¦hßè]w¿ã•õôVÿAGNbcu3FGL J1824.4+4310RX J1824.2+4309?ïü2~ҟá?8ÐUÛá`?>l	k÷5?8ÐUÛá`‡?ïü°þ(£Ñ?Q؉€hIi?:xºát"?Q؉€hIy?ïðl¨NGÞ?c‹—aÄ®?_&¯cpEÞ?c‹—ađ?ïÌÈYÙòÍ?j
@^ƒ"?y›Ó™Î?j
@^ƒ•4FGL J1824.7-3243?ç<"—´yÙÀ"V,UÉ`1À:­_ö	ÜùÀ<"Ó~—¶@?8Aºàf@O8œÿ¨?ь®¤˜¦*?Ùk¯#c²@	ŒªZ±ý>@Ùúf=!?ïʇ½ùö&?âtÒò¿â.ÂöŠ5y¿âcò¸ï 6¿ïôcê‹#µ?ïj¾º»RAGNagnPKS 1821-327?âHI7ö‰U?Ð)m—½t?ÛomíV?Ð)m—½t?ݓíe=Z?ÕFJ¬Ž:?á6}	MaS?ÕFJ¬Ž:?ß]Zûðl?¼ÅY™.à?àQR'}Ê?¼ÅY™.à?ÜÕÀé×?ÁVtM³âŸ?á•‹qó•?ÁVtM³âŸ4FGL J1825.1-5231¿ïn¨Û$À1u;÷'À9N\(õÃÀ;ä(ôëÐ@_êVËhÊ@;šû™hò?°Ù·µä?ÀªqK´´@Òµþ,Á@'dkåV?qÏJ*›Š¿ÙÀ.XØß*¿æ¸÷˜Rq½¿ãõՅØò¿êC7¢®–+¿ïÿ ºöAGNbcu3FGL J1825.2-5230PKS 1821-525?ïðM—Ý?WüKæ¤?_eÂÑE.?WüKæ©?ïû:ÿç)…?^nTèú?CcYî?^nTèú?îäa²r™w?•"¨[?¡¹äØÖh{?•"¨['?ïþÏQñ5w?‡z[—?#
à쨇"?‡z[	4FGL J1826.0-5037?ÁÑüdæÀ0Ý\…<ƒÀ:åCä/À<LERðh@ %ZÕHœ?ý͘T<?ËÏ?tN†?Çó(ªB?ýÒK&nÿ'@ݺÄâr¦¿ïþM"r›©?ïÿöÅĚϿ¬&SUȬ¿ÞøC¾EËf¿ç]þÈs¢¿Ñ‡wã¼RAGNbcuSUMSS J182551-503914?ïõZQ':?QlÌèf?UK]±‹à?QlÌèc?ïñðC¿-?v"ñ0ß6Ÿ?]úx¦¸?v"ñ0ß6œ?=?‡^{r'à?Ž]ÿ0»zÞ?‡^{r'à?ï&i€'' ?†tŠƒFҎ?›2ÏíÍÌ?†tŠƒFҍ4FGL J1827.5+2015?|›ꇫá@,X–Ý&·$À:ãAÒ2g[À<K§°³''@ N+9>ºü@	T!ÀD(?Ãߥ+Ï¿¥ú—$82e?ã|‰ˆª^
?û9ÐUîI?ïü!ƒÞFr¿å(Gýo¬á¿ãœa?`9¿ÚÑR+Sk¿Ñxâií¿íC·'sAGNbcuNVSS J182730+201309?ïö^0hn?UÑÐÊÌ2r?SCŸ/"ä:?UÑÐÊÌ2m?ïà1ρ?"­zIš?oÎ0~íbP?"­zI™?ïËÛû~ýn?'ã‹ U?z@J€?'ã‹ U?ï†$³wÏ?x%[<îz?Žvú"B?x%[<îx4FGL J1827.6-4029¿ÛY§ðÏßÀ*Q´þzÀ:Ås½fþ<À<Nx"PŒà@Q†QŒ@njCoÁY?ÐP¼›|GÏ?ÝaÅÂÂ\Ü@
•"äþòº@Xâš>…?ïùu'
5ô¿çumjf¦'¿Önà2…8¿îoÝÞm¿éÏÅÀi<¿ïÿ®¡hšôAGNbcu1RXS J182724.8-402904?îrW¿øØ?¯£Ád‡3Ü?¨ÚDr–?¯£Ád‡3Ü?æÃl©U?ÑL·ŒX·^?Òyñ&­Tá?ÑL·ŒX·^?ã~<ê.Ï?¹wdé/'Æ?Ù‡ð+¢a?¹wdé/'Æ?älÏ#1º8?µÇ£ Q‡p?×&a¹œ‹'?µÇ£ Q‡p4FGL J1828.0+2634¿É뎲™i@0ŽØ
±À;­î»4À<Žä†&ö@ ¬!®{}û?þ»ë¹!^?Ð ‰ãC0×?É87)Þ?ønã]2
>@¡€\[˃¿ïþR¡ªˆ?ïãë¸J_¿À®ŒDòMe¿áp ßs˜~¿Õj\|ؙ¿ë§A"4ØAGNbcuNVSS J182756+263313?ïéb8!Ê?cˇS?fñÇÞ6Š?cˇS~?ïô·¬§?q‡Õ¼;Ç]?WÜb𦲄?q‡Õ¼;Ç_?ïr¸"$Û?‹qå?'½û»d›?‹qá?ïRG`öÂ?'ê2
?•·Sá'¥?'ê2
4FGL J1828.7+3230¿ã&wᇜ@2Ÿl‹C•À: jüÎÀ<§Iˆà
ò@Í+4Ja?þyŒcP1q?ʜuìì'?äk•ð]Ì@–fœí@`Fë¡Ï?îé}'Ô?¯ ®ˏ¿Ö;™Ƚɿä…Lò!¿ïÿþó…õ?ïGÉÃ-ÚAGNbcu3FGL J1829.2+3229B2 1826+32D?ÆDñqMÕ?ĈÌHą?ênþ㬋?ĈÌHą?Ã[8ÑØ=¼?Ðz8ÂÛtœ?ë)1ˉð'?Ðz8ÂÛtœ?Å;ã÷Š;?®÷§H4D=?ê¾±q?®÷§H4D;?ÔÀÍðN?»C>áé†?埙Ø¿o?»C>áé†4FGL J1829.0-2417¿é©ÆˆpUÀäœ@=òÀ9M	1´®À;™Þ˜§+S@˜#wÔM@´¶býü?³ÒŸt¤í‹?"³n#kŒb?á Ϟ8dË@¼‰¿±Ü1¿åŸ'•¿†¿Ú##´e"¿ãhÆ]Gô¿à6U\Rç.¿êŒÕ€Ðtø¿š ½R¡ÛAGNbll3FGL J1828.9-24171RXS J182853.8-241746?ïkûÇí0?">!º:Ð?'€‡\ÙÑ?">!º:Ð?ïý:°
r?TCyP!É?6*¿¬q7?TCyP!Ä?î ±N+? üJ³¬Ç³?­ôï‹O? üJ³¬Ç´?︬éZ5¶?sQ"õì?ÔÅ©r'S?sQ"õí4FGL J1829.1+2729?æ}®Eº@0²{åS¬OÀ9ÄP¡C§À<L¥ËD@Ð<Q¿æ4@"îV,\?¼MfÿØ+¿?Äj´iS«¤@¦Ôš÷g«@ã·Shݺ?–tP›	Aƒ¿æ|š…R¿äñržƒ
f¿é¢>Çç¿ïÿ#–Ýýw¿ïúÚâ9EœAGNbcu3FGL J1829.2+273187GB 182712.0+272717?ï7UÙky?¢Òǧ¤zŸ?™DҐß÷?¢Òǧ¤zŸ?ìQ'©È‹?Ɛœ;…û?¿½v±»§?Ɛœ;…û?îR»©PÕ?Ÿ"-"(?ªÔEf*ò¡?Ÿ"-"(?ìn"›ž9?¤$_¬¹öG?¿¤‹[#5?¤$_¬¹öG4FGL J1829.2-5813¿èå	tEÈ&À4j½ãû½À8†‰À;–lÅ%8Ÿ@­ŽE'§d@rÑ®³Ý?œ€4»Í?ÀXƒ#á\@`^åh¥@
t÷"ᬿÑAwcä«ç¿ãÆ°žBö ¿èS]õÿv¿æë+Ý~uÒ¿ìIìqþ¿ïÿî' ÇAGNfsrqPKS 1824-582?ïí Ét¡Þ?aÙÛ@`¿Q?b_6‹^$5?aÙÛ@`¿O?ïñÖ/ÂY?qxp6€?\S {çMæ?qxp6'?ïN¸-íù?ÂýÌ~æL?–(úB@ݏ?ÂýÌ~æN?ïý¾þ'á?&«T"O?2hóš<?&«T"e4FGL J1829.3+5402?؏üö›eD@8Ìñ`®—À9úVÔ"+¤À<d?³t63@ 5q4ˎ´?û©Ø@žUÁ?·*KØñsJ?½Á"o:öK@õM¾Ñb@9{E¼D¿ïå!4y?ï'~ nö¿×—ñ"íjÒ¿Ö9ñ'õèO¿Þ‹}ÂM—ã¿â'«@‹AGNbll3FGL J1829.4+5402RX J1829.3+5403?ïýòß´œÖ?4U€ªÖöË?0i[K?4U€ªÖö©?ïø³5"ÙC?`'~AÒ?M3)°šû?`'~AÕ?ïæ³)›Ýª?hŸŠÐÒ?iLÖd"V?hŸŠÐÒ?ïÒ̹¿?xKi¯Žûˆ?‹ËLûQ:?xKi¯Žûˆ4FGL J1829.9+3934?ÍI"HbÅ@4ȕá~4¹À:Ðw/†FÀ<šã'áït@HK×Cô!@"ýØ?ĺ{B?·ÉÓH<ç?ôÿ5ºÌð@ê;ò•í?ð¿ä:'
‹þ¿å—Î=e;C¿Ù¦DÉ]­¿ë&i@‹`q¿ïånN'4KAGNbcuNVSS J183003+393638?ïñÐÙ49?_£ôY°?\^M—á‹ø?_£ôY¼?ï›gSãa?šß%½C/e?‰&+'»õ?šß%½C/f?ï¤b†ó?ƒ'Í%½í?†ÿ'^C<¢?ƒ'Í%½í?îhDùk*?‹»Ëà…g?¨	{°iMi?‹»Ëà…h4FGL J1830.0-5225¿ïS"ÓcTüÀ2ÁLf
À:É20Ô´"À<lý@´%@5ՈJø?ùÞ Ô÷=º?Ö%>}êª?â¯'9*Ä@Ü;\Í`q@@DˆE?íº¬Ùè>B¿ïÏÖÍ׏?î´ýØÞS¿×'Ï<h¼¿ìCÌÞj"¿ïüDôü–¿AGNbllSUMSS J183004-522618?ïñÂöã´Í?a}§x­Ô"?\z8–h?a}§x­Ô"?ïé«?Ês?…e~'ra¨?fTÀ5Œs?…e~'ra¨?î0ñ‰˜­?žBu6-R?¬ÿçfu#?žBu6-Q?ï2_—šÛš?Ž»Å<̼"?™´
¤Œæ?Ž»Å<̼"4FGL J1830.0+1324?ÈóÔsIx@%~`ÔV.À9é©óƒð»À<	‰±Å	Š@Ä{MSDö@SZðç^?ÀHjýÏÏ?±–c?{§'?ôúkÖ证@	€ãäky÷¿Ø´ªagùä¿ê–à·e\{¿à'mb*W¿à,&Ïw¢¿Ý:¤OÜ¿è‰52ç³ÙAGNbll3FGL J1829.8+1328MG1 J183001+1323?ïü£°'­?4xî]˜?:â{o'—?4xî]˜?ïú¤~Ç?d~!ÐMۛ?EnÄãü÷?d~!ÐMۛ?ïðXתÑ?fBÿ¥i!?_çNPª^b?fBÿ¥i?ïñšŽ£ ž?GI붹†?\Ê⸾Ś?GI붹†)4FGL J1830.1+0617?'OÙ£\/@Wáá1àÀ9<•ÃKCËÀ;‹PMö-@qV…sÈ@Ž£yè#?¸´¸ƒê…Å?·ÎFO?ü#ûØSÍ@z$n?ïÒjeÏg²¿Útî¿eÛý¿äÎ×ؙŠ¿âHŠèü®<¿êÒûºöás¿ÜÉÇÿÞrAGNfsrq3FGL J1830.1+0617TXS 1827+062?ïèe˜'?e`	2å¼?gúšêgoÝ?e`	2å¶?ïú\}30.?fŸ¥ÞÔ?FŽ3?E,?fŸ¥ÞÒ?îÇp6¹È?–ƒíNÔ?£ˆü"oƒ—?–ƒíNÒ?ïþý÷¤mw?U\Œ?  …¹(«??U\/4FGL J1830.2-4443¿É¢¯+­*=À.jÞe{"ÜÀ9BW@X¶À;é·B÷ÌU@'²^Ø(@L~ä­³?³XÚ©¯;?ͨœkÛñ-@Ú:_w^Ü@íÇBŸ6ç¿É6$ª.gG¿àG¯â0aG¿è¥ú?÷'Ç¿èeÞfRD¿í`b@fø¿ðAGNbcu3FGL J1830.0-4439PMN J1830-4441?ï´lfá?†€Ù®j‹?'äÿæG»"?†€Ù®jŒ?ïù•"˅?`¿ÉØMsX?I©ï¨Ñïô?`¿ÉØMsT?íŒìÌmrT?¡ùò°ËLÚ?³˜™œ"ma?¡ùò°ËLÚ?ïýý‰M?)YÃIÙ?7èµ—o?)YÃIæ4FGL J1830.7-2713?ïúÂå?´0À"jP
_À9—ìoîÀ;¨uÕo3@nƒGr°@b¢§_U?º¶ñ™4ïÌ?¼Ö€TÏG@<h€òÙ§@u•ßû¨­?ïŋZ;µ¹¿áýwå?¿áýÖ?<Uò¿ÞÊÒ É¤#¿åÈ¿nÀR¿ïþ؃ªDAGNbcu3FGL J1831.0-2714PMN J1831-2714?ﺩGWÎ?'\؟±?U®:*+?'\؟±?ìvÞL[ ?Äv'â*C×?¼I
"ÿ´?Äv'â*C×?îu^"Æ?œÒ«ý4`¤?¨ª¿³‰?œÒ«ý4`¥?é=Wélš?¨þ¯ßÀûÀ?ÉÃ
 ZMš?¨þ¯ßÀû¿4FGL J1831.9+3820¿è¨éj™øt@4š€If{À;Pz9'ÍÀ<¾Ýšzj)@ cnv*S¼?þ†Ôš÷g«?ÐFðù²?Ð2?"?ý,©@։å@'ԱÿîÂë'D"X¿ëöòoô"¢?ïþž¦ž»¿àԄ¡ºÐK¿è"PïܜN?˜bãz
b>AGNbll1RXS J183202.2+382132?ï×J9á	?såLí ?tZã9{È?såLí£?ïõ÷| &?w&ó"ò"S?TÛ¿µ¤?w&ó"ò"V?îò0&Ñð>?"íó
úzÚ? Üý'àü?"íó
úzÚ?ï£nã[?uõ×Aõû?‡>¤G)x?uõ×Aõü4FGL J1832.6-5658?à"]âh&UÀ4m?ž{À9d8F˜jÅÀ<"a+"@qƒ¯½@"+¶g/º?±œÅžbe?®±±à¯¥?ú*M`Ûâê@ÙFœF?ì.¾¯R¾¿åt…
›¿à4º-ô¿àP"AÉN¿å<YjÕa¿ähÁTɅðAGNbll3FGL J1832.4-5659PMN J1832-5659?ïôª-ƒû?UöÐO‡Ž?Vªý¤ø¶?UöÐO‡–?ïõÎãÍ?ucÄSÊQ?UÜb9òe?ucÄSÊQ?ïë1 Ìý˜?qºõ.([?dÎ_3h¢?qºõ.([u?ïmÛBn›³?{
7кž?'D—²,‰£?{
7к¡4FGL J1833.6-2103?íyÕòöÀѹ_1¾¿À6`°Å/JÀ:‰"ªNô@¸£Äë¬â@¦v§&J?‹­IòèÔ?¸eúéHÙ@&¬`gHäu@Aóâee¿Êg>ÀZ#¿ãÀVgâ¿çlë¯#¿ç%¼R+F¿ê>ùºì¿îö÷ãÑÌAGNFSRQ3FGL J1833.6-2103PKS 1830-211?ï¿·C¦sW?}h`X¶gí?€/c*–?}h`X¶gí?î(ý)ƌ¦?ÃÀ¯Š}
?­p-c—5£?ÃÀ¯Š}
?î(íS!Î? Òëٝ+?­w*Íã2? Òëٝ+ž?îefQH? ¥	g#?©©šîîkv? ¥	g#4FGL J1834.2+3136¿ìOp2²1@13¬)ÜrÀ:˜T+
pÀ<MAî·Ù @!6âågù9?þEäæŸê?ÌüŒ¥ä?²{;4´g¦?çu *­R´@ç™ZÚl?ïêõ6¿åŽü¢}mê¿ì›'û? \¸<ÇÜx¿ÝmmVD°3¿åÛBöAGNfsrq4C +31.51?ïü1ä42?=ï`rüa?>pÞ_ŽwÑ?=ï`rüj?ïôÑ8Ç­?sìsÛú{?V]ŽqÔ£¦?sìsÛúz?ïٖ¾ØÕ?vÝö(H~Â?s4 À•Î?vÝö(H~È?ï¤ü¬óþ¿?sƒÃCqy¬?†ÀÔÃP?sƒÃCqy«4FGL J1834.7-5858¿ï‹¹wNX±À4ñoiÀ:›ËáªÀ<6h¯ìÂ6@¬Bè2@'V¡ÍDÂ?Ð6Ö@hûÂ?И
M`Ûã?þV>J¾j3@	(#á≿ï_jÿR[?ïãyòÄ-¿åF;Šsâ¿ä&vVžrF¿îÚ"ö¥
¿ïþs£eË6AGNbllPKS 1830-589?ïâÂoöè?naœ¤(?m=€	ð?naœ¤&?ï÷+H_Œ6?h™­ÏÏ?Q©o@瓩?h™­ÏÏ?톭r"´Û?£&á"«?³Ê"kÚY)?£&á"ª?ïLʱ&™?'_Ȭál?f©Û,×?'_Ȭál4FGL J1835.5+1349?í>XÝ·@#pxú½ àÀ:^qhøçÞÀ<´-™–?@xD6¿@M|Š•?ʪ < ð%?Ç­NWPôº?ÿw¶4ÚÓ @ðÓQÌ%ˆ¿ïÞf"‹=?ï˜j$aY¿ãB#%žõú¿ØÏ= ˜ò¿å/¼»Ý'@¿ïúDŸlArAGNbll3FGL J1835.4+1349TXS 1833+137?ïì–åvåÆ?cµÊ'˜á?ci‰:º?cµÊ'˜áž?ïãfj"ž¢?‰Ï;'í9 ?l™•{a]˜?‰Ï;'í9 ?ïX
û¸?'<ÍÑ«?"þ\@ˆý½?'<ÍÑ®?ïyð,ò`?€§½G^e;?Üáúa´?€§½G^e94FGL J1836.4+3137¿èéWŽ˜î@0ÇQzF<À9ÃÈXÉűÀ;ã'‰±Å@·5ôƒ @ð%ï?¶‡Ü¾îy?žsÚÔ?å£|f'ì@	'tΉ‰?äPŽù,§(¿Ýùà4ì¿á)½h«»¿èŒö%‹«¿ã{6l£—I¿ÒS<}‰ÃŽAGNbll3FGL J1836.3+3137RX J1836.2+3136?ïéo(+'L?^ù÷û«
f?f×Ôسa?^ù÷û«
i?ïü)¯fX?Z‰0îa¤?>²"Í?_Ñ?Z‰0îa¨?ï?†¸7ÞޑÀ?ˆÝ½Ä;?†¸7ÞޑÂ?ïޘŽÉ£?\Ð&Üí5R?p³¸›®†?\Ð&Üí5C4FGL J1836.5+1948?Þ$9¶x¿@("'Ù±·žÀ:#GÃEeÀ<(¢¹ÓËÅ@tˆ$QC@ÖïÞIÌÓ?¼M3y…'?âmY09?ÓÌô9ù ?úJC*L.Ø¿ážf½¤:Ý¿æDw(U‰Ÿ¿ã F&Tþ_¿àËx¤V‹þ¿Þ╠Ž¿ã'¸ú‡ñAGNbcuNVSS J183632+195047?ïÖÚ¢o?kÇ1¨•}?tÀw®Èc?kÇ1¨•€?ïâæ\ÚM?†…ˆu2çÕ?m£%²þá?†…ˆu2çÔ?ïÄf[ä~-?}óqF3ð÷?}ÌÒ
Àé'?}óqF3ð÷?ï[7ã?'?€'—×ËcÇ?"™ø
æ?€'—×ËcÇ4FGL J1837.0+5347?×bL¢ã('@7£¾ýq?À:"
xÀ<nCe°^@n]ST0@Ê:KUhè?µ'éÀè+迅Ln:Á?Í+éþ5ûe@æ åhã¿ÔŸ¯=æÜ¿èT×È©Qž¿çõšÀ[¥¿ãXˆAØg‹¿ë>"_¦XÅ¿ïÿ˒:)ÇAGNbcuNVSS J183710+534704?ïÖüŸA¯?sŸéÖ²Âþ?t°_(xä?sŸéÖ²Âþ?ïû	±†?Z_Ә—É)?CÚ;©íó?Z_Ә—É/?ï‰8À÷?Š)C^Ã2Í?±úO S?Š)C^Ã2Ë?ïÏ-iwi?g@â¯•?xiKDKË?g@â¯œ4FGL J1837.3+1052¿ï-ÆP©8@ '5ø	'À9ÙúàŽµÀ;±Àn¹@gýY‡…Æ@b<ççÛ?ÕvŸC§ ?ÃQ]?ÌÐ?ÿºC'œüû@9C!ór?š¾\È¿Ýà鄓x¿ê/·éùr¿âu>`bì3¿çôñ^|¿ïÿûÎBÓAGNbcuNVSS J183713+105143?ï¶ÿ&V9†?†yLn"J?'@6jqž2?†yLn"J?ïö¯µü@?mÄÞ>õáx?Sƒ‡?mÄÞ>õáz?î	Ñ0Î{?¥ðY!°?¯bìóN¹?¥ðY!±?ï´
áhŠj?m4ßdÒP?'ýG¥ÝeN?m4ßdÒE4FGL J1837.4-1646¿è…gejÀ9åâGˆUÀ9šsfÿéZÀ;úý9@.Û'X‰"@¾+Uï ?ÕOƒ3є?åAˆËëü=@R
Á‰¢¬@å?ïÞþ"v¿ÓtnÒE²'¿è<Ÿ9@>¿î¾£%¿ïÿÿ)@k*?ïøš°ðÎ4AGNbcu2MASS J18373301-1647530?ìŠûó…€Ã?Á?œøúÞ?»¨ cÓùá?Á?œøúÞ?ëoÔ?Ë1óÊWÉx?ÃÿÆC»Ä¬?Ë1óÊWÉx?âê|P¨e©?±â%ñêVÇ?Ú+^¯4­?±â%ñêVÈ?åwÉô›£÷?½[ìâÏÀ?Õlȸ?½[ìâÏÀ4FGL J1838.0-5959¿çîiޒ`nÀ5¦¾zúr"À:®Èú°4çÀ<~PŽÌÝ@ ÀR¬u>p?ùÒk<Žüˆ?Ψ£!ؗÜ?Òw¬tg°é@ò¿-§Ù@¦žûn¿è›¤¡4˜Ž?î(ø|}ÿà?è7é{Y=¿ÖXF½ÿ}¿á\LœÄß¿åPŒ?>qAGNbll3FGL J1838.5-6006SUMSS J183806-600033?ïÜÏóH9?vBö#Åè›?qñ[ã‡?vBö#Åè–?ïÞ	ó@ª¾?€?)Ï^X?pû_ª¡D?€?)Ï^T?ï.ãk<Œ¼?" õÌÆLÏ?š#'˜nh'?" õÌÆLÏ?îý2™þj?Œ8†/ø? ,Öoa?Œ8†/ø4FGL J1838.4-6023¿Ûk]œ'‹À5Î/ßÁœÀ;Â~•1UÀ<™7¨ùä@!aéÆ,ʎ?ý¹Y_ç?ǐÈû"?–†¾(LØÔ?Ñcº¥@·ä$\V?ïå$|·
Ä¿ä¤ßßÏ^¿åOV_2?˜¿ÖE@[º»Ó¿æêNˆ#O¿·ø'wAGNbll2MASS J18382063-6025224?ïÿ»6ƾ>÷UÈ´<?9òNPOÞ>÷UÈ·{?ïþHó*Ê?\Ò¾>!?/;pÍSm!?\Ò¾>?ïù#Õ|Oô?fEßo¾E­?KpªÀ/Ô?fEßo¾E¶?ïúac›¥ð?6ƒ{kÎ[?Fzq'hAÍ?6ƒ{kÎn4FGL J1838.8+4802?"|Mx¼ª*@5҉üm¤HÀ8Y…O_¹¤À;'*è´@¿õ=Ú+/?ü9"ù÷¨?¡Dª©â< ?§Í?¹Ss@¢ÁE°
y@#3d1¿ÓbÛ, Å¿Õà¢A³Õ¿à-n}ŒÙ¿ÔhrÛâ`¿à¡u0.¿ÚÍÒ»ú²AGNbll3FGL J1838.8+4802GB6 J1838+4802?ïþwUP?!öGÁy£ ?(ŠªþqY?!öGÁy£×?ïø4y©å?qždšT%í?O/¶Xj2?qždšT%ð?ïä)Þ³)ú?q»Ê²б?kÖ!LÖõ?q»Ê²Ш?ïÿ"¾AŸ?"¸Vº\?Ð_¯˜K?"¸Vºt4FGL J1838.9-3457¿Ñ¬®W­8À)—¬>·Ë´À:NÒàD²À<DÀ:î˜@#ݤ
‹Ê@®È b?Ä	çƒÝ?ßa¯²à'|@Ž6Kìg@ðÜvü?ïø©"¹`?»-(­Z¿áÌHþv"¿çà,€f—º¿ï¦tÞÏ-пï­ðÔ+AGNbcuAT20G J183923-345348?Ÿ	éû"±?¢_¯üH?ï·ø°#Û?¢_¯üG?½$(>–[Ù?±†?ì[zø-4…?±†?¹‰Ž-´•H?ªâÂül
ê?ìÎÎ:ImX?ªâÂül
è?Ï£!ÓeŸ?©Bµ{²%ž?è7‹8f˜?©Bµ{²%ž4FGL J1839.6-7107¿ïŽ¾O£õÀ8ŸØ­«ŸVÀ:ƒñ'¨4À<l'ÐR@&ò	GQx@a<á1ޟ?Â6‡»öÁ?Ño^|âÿ"@ƒ)›üå@J肊ßB?Ð%óD/Ú¹¿æ*#ŸÂR ¿ê܍YýL¿ì\e'TPº¿ð?ïÿÖ°cAGNfsrqPKS 1831-711?ïúˆÁÁï?OŠ›b
d?EÜøùÀB"?OŠ›b
m?ïôŠ4k_ï?‡«7¾¯¾ü?Vë—)@"Z?‡«7¾¯¾ü?î<JÕIè9?šO'ù¾SQ?¬;R«a|h?šO'ù¾SR?ïõ.®î#?Kʯ &i?U¢¢#Ó»z?Kʯ &i04FGL J1840.6-5545?êÌÙYÌZýÀ4²ôàM/À:"µÄr‹8À<95>»@N©•·b@i¦Âwu?ÌF³Ã'dÂ?Îå=F‡xÛ?þ{ƒ@GþЪýÅ¿¡1=ßoοÚ]7þôè¿êßß~€8 ¿à‰T!ÀD(¿ïþ_–}Û?ïÓä^
ýDAGNbcuPMN J1841-5544?ïû½ZR‡?F¯ñ-ÔH?A
–µã¤¤?F¯ñ-Ô`?ïþwji^?B7ÄÆϳù?(‰Yh
‡?B7ÄÆϳí?î¬ÎüÉl¤?˜T½_µ?¥33i5·?˜T½_²?ïÿ¸³­öÈ>úû>Ràƒ ?Ó'N>úû>Rà'4FGL J1841.0+6115¿ï¾¯¿äá@8ÉzÝð,À:+ª¨µ–À<"˜8p‰Ö@­Z—@iøÂ!?¶e Ÿa¿"HóÜ'«?Üùm'e™@šš?íˆZ吿çs×¾}J¿ë%§>Ê¿Òft©H›¿ê|•aütZ¿é‰@»±òVAGNbcu3FGL J1840.5+611687GB 184000.4+611120?ïö¿}"äO?R«U×¹@?Rö7a¨?R«U×¹<?ïþ¤4?Hº·e
?/…¼¾ïþ?Hº·e
a?ïÁ!Hn¤d?€S©Ÿg?o[È­Îg?€S©Ÿd?ïýËfí?*¹†3¤òŒ?7Q§ÌÈ¡n?*¹†3¤òt4FGL J1841.3+2909¿Óg°Òˆ7»@-±«ŸU›=À:Vî#^ªÀ<)Æ°Sƒ@!ÏYè~¯?ùP¬:†
Ì?Äd?D¹mt?ÃÄ©Ü¡V@nÊhn~c@ØíÙ6èt?îæ{_ïJ¿è±Š¼‡l¿Õ"!'—ô~¿Ó«é]&KÄ¿ÁƒZèÙÉ¿ãúM~caAGNbll3FGL J1841.2+2910MG3 J184126+2910?eƒìg?"ÙÝݪ™µ?ˆ'æŸåÞ?"ÙÝݪ™´?ïͼÄ*Sž?'~Ëw†Fg?y!êÖ0÷?'~Ëw†Fg?îÛ[NI5?šs0Ÿ¿0V?¢JKûl¡?šs0Ÿ¿0X?îˆÚk‡ž:?"Ëóé5´Å?§rYG†y?"Ëóé5´Ä4FGL J1841.8+3218?ËwÑþÛæ`@/ô(²¦°ÙÀ:&jö±À<'-Z¬@ h–=º6?øå'Á(?È-Š½2Ðã?ϓºÝa @ËýÝï@
¹é¹S?ï×O!¦Bõ¿ ´T0ý¿â4»ÉoJ;¿£\|$56¿ÙÕÁ½ú÷Ø¿êÒ]«AGNbll3FGL J1841.7+3218RX J1841.7+3218?ïÍvH{Ύ?wê´Bgs?yDÛ¸T?wê´Bgq?ïö€a
N¬?eZ8¼¨`?Rÿ=åb§Ü?eZ8¼¨_?íÔՍ£?£—à‡Ot?³ñYS'çÜ?£—à‡Ou?ïâ^öùµ?Y{¸GœÐï?m¡ì	JŽ?Y{¸GœÐõ4FGL J1842.3+6810¿Ú&ÉՖÜ@9à(=5ëtÀ:5óÚó×À<FõÉEXÐ@"ø4.°Ã@.d"Õ?¾§à?†d?³?ÐÿŒh?ñ{½•ø$i@ëóbål?å}>" 
Q¿à²ù¢í]¿çýªðÙòO¿çV²X­@¿åÿ~?ËòÝ¿ïý:ˆ'
YAGNfsrq3FGL J1842.8+6810S4 1842+68?ïúâíT:c?@CÈ2
q"?DtJ¯r?@CÈ2
q¦?ïý4*¡0\?Lt¦nó[	?6^ªö}@?Lt¦nó[?ïãóíژ¾?l}`ŸU«e?l%gCT?l}`ŸU«W?ïÅ7§Âk?gk!e¡?}du,ʀ?gk!e¡
4FGL J1842.4-5840¿æY—$s•ûÀ5Í!…Æ~À:'FÙÙ$ÊÀ<kÕW2@!ßX6øº'?ùµ>U¦$Â?À¹e¼ÈGØ?³ÒÈ ~vd?õÂäßJ@c?cÃ÷¿ïv³…Óé÷?î϶¡'6y?¥'@"ɝ\¿Òëý?Ò¿à±6¤û©¿ÇNògHºAGNbll3FGL J1842.3-58411RXS J184230.6-584202?ïÿ˜gÓ³O?kHªí7?	æ,M?kHªìo?ïþ&=%##?F"{È?-œ-­ÍÓW?F"{»?ïö–&¸#Û?Sa—¼â?RÓ²¸Kd?Sa—¼â?ïýv¥Ø>L?+Ú²‡¥çö?4JÑ>
©Ý?+Ú²‡¥çÀ4FGL J1842.4+7613?éŠ*LõÑ®@:ўùTëÀ:þ•{&çËÀ<zŒç¯¸@ߖK±YT@õ"yŸ(O?ųoC.ÓÓ¿±pþöÌ%?ꖝ^Ë@ÐÕ¹ÛX?âTO­¿ç`|wIãy¿èHèÜÍËпæ¸þ˜¡Í¿ÖÎ9Ì¿ïúµ¾=gêAGNbcuNVSS J184225+761046?ïûa&dã?IjÉ!Œò+?B{gŠlv4?IjÉ!Œò?ïûg/­Ýx?bI¾Bá?BcAHŠú?bI¾Bå?ïË51I5?~"²§0'?zegrÛe)?~"²§0z?ïõ–°°-?J€ŠÕPº0?TÓôžŸ¥Æ?J€ŠÕPº64FGL J1843.4-4835¿®Üd̪·À2Ág#$È6À;#jJ µ'À<"Þ·°ÛÕ@ /(Œ't?ÿŠ"¢Óä?ÌGOŸÐjf?²ÐË_ƒQ?꤫`kz¢?ù!¥AB•?î"þ×áÓÅ?ï™G™ò"í¿Ô'd=AT¿éÈ»ÆKç?ÊSk¢ep¿ðAGNrdgPKS 1839-48?ïüy3dLá?J¦¶æb§?<6dݙ=?J¦¶æbª?ïì硏'ô?ƒ
ê}è
?c^p}´?ƒ
ê}è?ïeÂ'æ?‹>Öôð-|?"G¿ÿÏ£k?‹>Öôð-u?ïg®9ÑÀ(?‡J"zzy@?"
8ÅÇû?‡J"zzy@4FGL J1843.8-2011?¿:Ê|~ÀЃn—À:§\ŠD'À<\W=Ôvå@Þ^eþj@Ðg¤T?ÎÁ#vQÁ?â":Re@ÚÙºñØö@ÑË«`?ïÿ΁ز´¿È=䧉ò2¿´l¶!9¶…¿á[ā¤°N¿îɟ†B¤À¿ïôÒÛÇ5AGNbcuNVSS J184339-200606?ãï[;ª<?ÌÁîG-˜ì?Ø!Iˆ«‡Â?ÌÁîG-˜ë?àvr)?Óá¦"	?ßõË­Ö?Óá¦"	?Òë&Ùˆ?Àz>žßý¤?æŠlü9<?Àz>žßý¤?àd¦	ã#z?³-'É\Í}?ß6³ì9¹?³-'É\Í}4FGL J1844.4+1547¿æhmádé@!DqæÍ)À8¢Ž`€sXÀ;[vý^ù@ó%~¿£™?ÿªúêí?ªÿö3á?¸¼¨½Mþ¼@/½jY:.@£‰Ê™–¿?ïæ(S`'¿âzŒŽ\¿Ù8i}òõ¿Ýx6zæP¿äXÅÉ£M¿âØ€_5ðAGNbll3FGL J1844.3+1547NVSS J184425+154646?ïþ'Êß?("¼#é}h?-ƒ^®'Ì?("¼#é}è?ïæúK¤è?'1÷æ9?ir´[C?'1÷æ=?ï©îSìqã?‡@—vw>-?…"kã‡G?‡@—vw>)?ï´¥æ®*?k¢Xóö¬?'Ö†Tu{ƒ?k¢Xóö°4FGL J1844.8-3248¿éõô˜:bÀ*)#å¸VÀ:ßT¦Ë±À<VÛÉ¿Ò@ çk $|?ýƒqÚ7ï[?ÌBûRFI?ÁJ¬ ¯Íã?÷<c'í"Ó@¸c3V?ÝØ̵O؅?Ù›ÍÀ"?ï&;Óë¤ÿ¿ÔÐ{)Ðß¿ÜöØ9™…¿ç>¢ÉAGNbcuNVSS J184445-324641?ïõ}Ó
÷?Rþ·žÙCp?UYêɁ?Rþ·žÙCe?ïóš$Ǩ‡?wÑí1Ì:µ?X˶p®ð¦?wÑí1Ì:µ?ïà~öå?s²‡rv´L?o	ùû¹?s²‡rv´J?ï%ÉÀ"où?Št³Ò¥]d?›FÇírÓ?Št³Ò¥]d4FGL J1844.9+5709?ÔþD]£¸"@7`ÿ—$tTÀ9æèˆêõ­À<pOŠL@ŸÍ¾G[@h§¤WÚ?´Jßø"»í?¦³À¿Ö͵?ñ"wXüñX?û`gô°ì¿æX¨mqób¿ÜÀff²g¿äiÿöÅÅ¿à⣘öÜk¿ãö"¡¸!¿èÖNUÎAGNbll3FGL J1844.1+5709TXS 1843+571?ïËûäß±?ný‹ŽÄî?z
'F?ný‹ŽÄè?ïo–¢-5µ?¨kƒë¥ì?'
+ºYI?¨kƒë¥ì?ï˜	÷›"?"ó·º´¿?‰ý'øâ?"ó·º´µ?í|\Œ?œCí\ë?´‹Â-¯?œCí\ê4FGL J1845.0+1613¿íúš;òŸ
@!cåÙä"À9Ñ°C)J|À;‰ôRLÓî@+³Ö0Ϊ@ïsÚZT?Àñ®X˜r}?§;ýå§?é^«QR+@ç;2±A¿ïü+ഐ?ïû4SÄ£3¿èe­¤™`¿åøç¨eݿᆌáû2;¿â‡¹1åUZAGNbcu87GB 184225.9+161105?ï%G8HÄá?šs
zlv?›WöçcÜ?šs
zlv?ï¦@
a"f? ÐõÍc¯°?†oýgšæ=? ÐõÍc¯°?íXW4, ?¦v}(†B?·-=F^žÿ?¦v}(†B?î×Ú —™?'ÁzYãó?¢'Uööz?'ÁzYãò4FGL J1846.7+7238¿ï ½â¡…@:%9C¬ÅÀ;r«¯EÓIÀ<õøٛi@!‡Ý^?{k?ó|tðlå?ßÀç,¬0?َޖxÓ?ÿ›x¦@ÿm[M-°?í[Ý¡[Z¿îñÄhz<Ý¿Ñç3À̹W?Ú¶ÁÚUv¿Î0¥å,j¿åÐîš|îhAGNbcuRX J1846.1+7237?ïýoØIåu?3Ž•`ÕÒ?4=°ÔO‡?3Ž•`ÕÒ?ïýÀ÷¿í¶?JŽÝ>\å?1øB'TÃ?JŽÝ>\ò?ïÄoxÆ°¹?€(—Ž4õ?}ÈCœ§¤?€(—Ž4ø?ïüï¹Yy?0T…·*~k?8‡Ò54Bh?0T…·*~c4FGL J1847.6+5219?ï¿T•Ø@5¶–6—lÀ:ñXeò£ À<¾ÿ
6º§@ljßgY+?ÿ̀CRe?Ðc"GÁ`?Ð	ZÝN@XCùTT@z$'±rÿ?ÛT9}¥Z¿á*¥Å÷Æv¿â&©ý¿ÞÓ¿àÐ×ôH;Ù¿é¦n£KÊ¿ïÿþÞ÷AGNbcuNVSS J184754+521513?ïï>Sd>»?_ûµ6Žõ?`Á¬›ÁF@?_ûµ6Žð?ïê5Íâ
ö?'üï‰Ò'?eÊ2ò
o?'üï‰Ò'?î§×ä©
?š2ê'ð±Æ?¥'µo/
?š2ê'ð±Æ?ïjÏÝì¢á?vøoÀ­O?'¦Bk£í?vøoÀ­P4FGL J1848.1-4230¿¯Ö⫾rÀ1_󾩛À:Sˆs©À<(ôB\›â@Ä:P]æe@‡zÛ?¿e')]œh?«$|a$ˆ ?îVužèŽ@ø`ÍöŸ?ïöðÂuZö?ÓÒ)-ó»¿é¡¿ØȄ¿á|×­O¿æEòèn¿ÕÏ°¬AGNbcu3FGL J1848.1-4230PMN J1848-4230?%QÍ-?ŒÒ*Söº?—¶«Œ´ä?ŒÒ*Sö¼?ïÝ´»k+?Ù¾z¼?q%¢Jjtg?Ù¾z½?ï=ìêdÉ?'ª°…Äª?˜Bb¾"fÊ?'ª°…Ä­?ïH–(±?"q¡j?í:éÅ?"q¡j'4FGL J1848.4+3217?æCò{'`@-_r'Ä"BÀ8'ÞѲÛÀ;il«$@#åÓ©‹@B[úҙ•?®(~îÙ£?Ç5Z«'@ó<£~@ŠÂ'4›¿ã'—|ˆç›¿Ùl`üD3·¿â¤«ã¢Ò¿ç皮l¿èʾ­	c¿ðAGNFSRQ3FGL J1848.4+3216B2 1846+32A?ï6Ÿ æ¸f?°ZéâÍ2a?™,ã(ó@?°ZéâÍ2a?ïëu€f?{Œ¯˜áօ?dîŠó›?{Œ¯˜áք?éÈüvxg?°^"šÙÐ?Èߐ&e?°^"šÙÐ?ïöãUŠý?E~"``Q¦?R9TëÊû?E~"``Q4FGL J1848.5+6537¿²ªÖ©´ÀE@8Õã§Ú¤ýÀ;1CºióºÀ<Ú!›[:¹@!'³­Áð?øçKƒŒ?Î2Sº<Qj?ÆÈdȬ©?ûõÓ £äv@ö{¬ô•>¿çW>«6z¿í²1«s¶±¿Ì"Æv)¿Á!JÓbé¿Üà4óý">¿Áº†ú¾VAGNbllNVSS J184822+653702?ïÿ8|n È?Y'XM?ðr+ç_?Y'XM,?ïý¦"€?L؇P×dó?2Îïÿ›û	?L؇P×dê?ï裀魗?pÕ !¡i%?g\Ri¸?pÕ !¡i!?ïüQpÚÔ¯?.ÖU¦Ü|é?=ty)Z‡r?.ÖU¦Ü}#4FGL J1848.5+3243?íÍícSj¯@-¦¥.ùÏÀ8oSö!YíÀ;®»iÎ@hé‡B©ô@ß=?%°?¨iäöd?º˜»Î!á|@`ÔV.@¨ê×ÿ?ÝN;Í5¨¿ã9€hÆ¿æ‡Íôêù¿å';C¢ìÿ¿èÐÀ⳾߿ïþ¶ôô3CAGNfsrq2FGL J1848.6+3241B2 1846+32B?ïõrz€?OvE¡ôô?Táý‹?OvE¡ôÊ?ïñ—M¼?uÁŽ;
ȏ?]öÑeð‰J?uÁŽ;
Ȑ?âR?ª?šÝ' áß?¦&¡ÚÜ\?šÝ' áâ?ïõèïeÍ?EœôxÓ	5?T. Å4cB?EœôxÓ	(4FGL J1848.6-2711¿ÎRëYƒÀ&é§~^ª°À9éà¸<À;¹á`x@_ß4ÿ@S{š«'?ÊÀ	šÞ?ÓÈ5Ä+m@OÀ1³×@ÂMò§'¿Ì"ö%j¿â¼è‹+B¿è±`Ëò¥¿êétšпïþظ"Yä¿î…§ß­z!AGNbcuPMN J1848-2718?ì¦ò•Ø?»Õˆ"6w3?ºÈkQ?Ç?»Õˆ"6w4?ìuŸË+"?†¨Á!‹ï?¼S¦£_ý?†¨Á!‹ï?åîâÙ¡/?µ@é,*Dµ?Ô#Ì:L½¤?µ@é,*Dµ?ê5áçȖS?©¶ò<=‰?Ç(x`ݦ°?©¶ò<=Š4FGL J1848.9+4247¿ïÿ¤cÃ÷3@2wiDg8À:"~ù˜À<…uôxãA@ 2N@CRë__?ºÜdÅQƒU¿{^^ÞßS?½õc|@ê#sw›î¿ï꽟ˆF?ïÿ–þߙƒ¿à&D7guZ¿â0"!'÷¿¿Ü6^`Þg)¿ÔÄʟËãAGNbll3FGL J1848.9+4247RGB J1848+427?ïü¦c"¤t?<–ƒá‡æÙ?:ÌæêÜZ°?<–ƒá‡ç?ïü`êw6ì?W‹øKÐ#?<ø¬FH§0?W‹øKÐ#?ïåRðÈ0<?tŽ&d~?j­7ÏÅ6?tŽ&d{?ïòŠ´^°,?MÓD8Ã?Zê—BŸ¦~?MÓD8©4FGL J1849.2-1647?Ø«®@«‰œÀdkA—zÀ9Ä/µÐ1À;áRƒZ'ô@! •ÀR–?ÿ³LØç?³Óc"ÏÛJ¿¡t=‹Yn?猪Œžß?Ø0=³Gs:?ïЍa'^¿»YÓ0C)¿åè°;Ä|¿à¿…òèn¿Ø=ÏCtžã¿ËpÀ•ÆAGNbcu3FGL J1849.3-16451RXS J184919.7-164726?õ°¥x?ºlUë8@?Ž"Ö¢?ºlUë8@?é'ùø
ø"?Ñë7ôœ ?ɸÔî?Ñë7ôœ ?ï|½.œâ?‡H^IE4Â?hZ<¬c·?‡H^IE4Â?Ò!c™~wk?¶8õéßþT?æïN3@ÄI?¶8õéßþU4FGL J1849.2+6705¿ïØÙøƒ"@9
ǸÕ¦À7×Øã["‹À;"1ί%@mvK½Ä@Äù¯"?"œÃ"\©Ø?¸'t·7_@""ÇSçá@EŽŠ$¿Êƒ]Âþ¾¿à.ë¥Õçÿ¿ä»ð¶ù&¿äâ1ƒ/ÊÉ¿è	}WC´¿é%¥á¦x¥AGNFSRQ3FGL J1849.2+6705S4 1849+67?ïà"ïá
?jÖPA–è¹?oÝ<Pó?jÖPA–è»?ïÖ3¤TŽž?‹8߇Mpø?tæ-Õ¸°À?‹8߇Mpú?ïy™Ç/Ռ?'Þe?ÌÇN˜?'Þc?ïê0'ð?]³ÔKÖ?eÏmïäÀ?]³ÔKÛ4FGL J1849.3-6447¿ãøGÄå À8&A€ÓÏöÀ;+–^{¶À<¼…"êÔ@ æõ'çôp?ûyüE`\a?Ð˜'\?Ï||¨G1m@BؤU@wHÐöR?½ðÊ1u?ïãNÿl‡=¿åÊÁžpn¿»¼$^@|¿Úœ=£N¤(¿ïÿú Âî'AGNbcu1RXS J184924.8-644933?ïõÖØ
ü¥?Tée;§¾§?TROê¶Ý?Tée;§¾«?ïå:l²‹a?…¢²
[­V?jœMtžÃ?…¢²
[­V?vFÛ?"iýõ‹šÇ?‹ânI;_?"iýõ‹šÒ?îð:¡?œŸFQÑ? ÷®lUî?œŸFQÒ4FGL J1849.4+2745?ѽZ*|¡J@)U'Í}åÀ9÷ö•3À<&/Ta"@^dŠ$\@¾‡Ó[?½pÛ	{~Ñ?ÀÀç¦ÂÌï@Ü \–ÙÌ@e£zîޚ¿à«Ç>B…â¿ÚC¦³]þ¿áô.`:¨H¿ç
áŒR3¿ä•îê.¿ë¬ížÔkýAGNbll3FGL J1849.5+2751MG2 J184929+2748?ïÜËÎ÷…?q®Çã
Ñ?qš"x=d?q®Çã
Ó?ïøƒuª@Š?kàÛîþ?Mò)VýÐÄ?kàÛï?ï—ï
åƒ?ˆŒÜ–ãÓ?Š=yŸ±?ˆŒÜ–ãÐ?ïà[2'?WîZE0¹?o¤Ímî	?WîZE0°4FGL J1849.4-4313?às
Ít'êÀ1ÛV†''À9BT^üå™À;Û[Z™ª@Ú`	]L@úéZ¢
?­	*ÃoxU?½[3­VÚ@Kèÿ2z§@¢ç÷ ?ïÿã°> Í¿ÙAf|·¿âÃ{_œÈ£¿âAb ß9¿é'´þyî¿ÑM`pƒÛAGNbll3FGL J1849.4-4312PMN J1849-4314?ïöŠ•Ž€…?Vuýf`m?RêÔâþùG?Vuýf`e?ïæžÖ\cE?'±dTìQ¶?ia)£œ»?'±dTìQ¶?îô²?¡+¦Œ'?¯€¾3Þ4ê?¡+¦Œ"?ïp¬Âø«f?wµÜâÏ~?'êg ê"m?wµÜâπ4FGL J1850.1-0758?ë<»ë
ÓóÀ
½œtÜÀ9£Y7©ºyÀ;p]j>b;@'"ß @!ñÂO›I?¹f¢vb¿Ÿ 6^êNÆ?æ§VPn­]@羊êª-?퓢¿]"›¿è^ï^Èt¿ç}1¦¿ó¿ä¯'Á8¿ã€!ß&¡¿'
©¥š»AGNbcuNVSS J185002-075842?ï¤J s(j?'¶žKj#e?†íWã5å)?'¶žKj#e?ïù½‰¹é?] ±8æ?I	Ùð[ô?] ±8â?î"÷?"râ¼yÞ?¡t6ÏàŽ?"râ¼yÞ?ïiÚ@³I?}硪å1½?'Ä·ýI–ñ?}硪å1¿4FGL J1850.5+2631?îüµ}ˆ‡³@'ÛeDþ6ÒÀ:¹ß[DÊ4À<bèn@"¾×M.\	?ú'ðßьO?ÄÃô÷cNY?«ˆã$8U?çF߂±öˆ@ªöŽ<C¿ì3q|D=?ïϤîar¿Õ—"{ªñ0¿ØGt^4¿¿Þ²qA`Èm¿Y7ÕÀwAGNbllNVSS J185023+263151?ïý‡×Ê i?/O'à&n?3ÁA®ü·)?/O'à%ñ?ïö8Ð9`
?i"Oåbß?SŽ_?ê&?i"Oåbß~?ïí³oMÑ?c´³¨~ûŒ?bL².æ'?c´³¨~û‡?ïwô‡±?ƒï«bÆ¢š?'l_o	Ì?ƒï«bÆ¢š4FGL J1851.5+3406?Ø@ýS–¥×@-šÀY!À:;ţàÀ<n}'Þ[@@+0Û?+@Ÿ¼?ÈU…2à'?¹'8©ê ?ïf='u^@vwŽ
?Мöÿn5¿ëäa>y¿šW'Yb¿èÅŸ,«…¿Øò»ÈB¤¿ïõ‰ŸP'ÀAGNbcuB2 1849+34?ïû¯†´Ã?@,>¿¿?AAå,ó¸6?@,>¿Ð?ïüŠêÚ?`¬ÙÆl;ï?;¨¯9/ØÂ?`¬ÙÆl;ð?ï×P¨NüD?yËÈcQS?tW«ØÞ=?yËÈcQH?ïòÏUÄÐ?Hã†í·{?[ÖaTv_E?Hã†í·€4FGL J1852.4+4856¿ïò)̒æI@3òÜ]cˆfÀ8ä
kùMÀ<+ÑÁÿq@±à<Á&{@ï"b*˜?£&b•K3?ª†·>Æm@à5z5PD@&NIºO¿½6‰©âg¿áŽ­½gÿï¿å§|æÛkÌ¿áõÁb¶Y¿å U—¿ìÝ5Мe&AGNfsrq3FGL J1852.4+4856S4 1851+48?ïý?#Ú?0‡*_ÜШ?6á/œd?0‡*_ÜÐj?ïö¦îúì?yzÄ[<J?R³à"
'›?yzÄ[<E?ïÔHáä?x#/S`Å~?uðñۏ?x#/S`Å?ïÿ»Ë*>ö#<=ku??5Îî>ö#<=o™4FGL J1853.8+6714¿íç¥×½9T@8£NÛʗÀ;@8
‡=À<OìTR@ z}l@($¹ó¬5?Ò¥Y€ÏÉ,?Çrç~(úË?óµZ¥hõ@‹ÒªÝ8Ö?Ò/£#Ü¿íheå7&Þ?Û5ÚØS>¿ÜóA«›ú¿ã€;ÄÒ,ˆ¿âùZ"¡UAGNbll1ES 1853+671?ïØ%³ qý?r
Y‰à?sí&oÇ'?r
Y‰Þ?ïøZ-Î"8?o¶|¦ãÞ?N—HÇw"?o¶|¦ãÞ?ï>³1®½?"ìÚëè†P?˜=)™Ê(m?"ìÚëè†R?ïo
W_
Ò?€mãr}?'U¥É?€mãr}4FGL J1854.6-6007¿îÏePî¢cÀ7®Ý&·#îÀ:åùrGEÀ<¥¸	â@ù&
s±?ýâEîÑ?Ðd!s€?Ñ3©$Ññz?û¯É†Ç.þ@ÖQ·'¸­?înkón!¿ì·¹ª±?âP¤'ñ߬¿äqÎly¿àNQ!/Ð}¿ïþ\ÓAGNbll3FGL J1855.1-6008PMN J1854-6009?ïôb6fë?T#;rð×?Wÿ;"2)0?T#;rðÒ?ïøã#¸P?fìȃj?Lsqνý?fìȃh?ï'ʈû??ë=Õjëb?œ[®à˜%?ë=Õjë_?îïO:|?lú¦.)?¡X?¯È?lú¦.(4FGL J1855.8-2028¿è‰%Ž2KÀ$<âó¾ýÀ:ÍËÕVJÀ<>¥}Ójv@8£ÆCEÐ?ü{"¤£?Ô%ߙX+?ÝÎÆâ}
G@¦ò¥¤i×@	%rÒ/6¿éŠ"XŸÔ?ä¸Q€%TM?î¾h›Œ¹¿ÐDHÄ¿ã¿éåBnºs¿ïüHOúêAGNbcuPMN J1855-2027?ïö¸šŠµÕ?TJ´M·LE?RŽÊê"Ut?TJ´M·LD?ïô…\ÊRÅ?vl‹b)h]?VõFkZw›?vl‹b)h`?înW\¯?ŸnETªFÂ?¯™Žº5?ŸnETªFÄ?ï³j]'	?v46WÞ|?ƒ%[è¶=Ó?v46WÞz4FGL J1857.9+0313c?ÙD*Ñ=Ù¢?$yςgÀ8€Ä0FéÀ9É瀭9Š@󾑠¦Ô@oÃzn?Ô¨(÷?ф(£ãž@	oŽÀøƒ4@ˆLôzeÍ?ïM›^•·¿ìMè@EÀT¿áÁcâþ¿çª.£ˆ0¿è°KŒÆL€¿á_#a.AAGNbcuLQAC 284+003<?Í—³ïô?Êí­ƒ4 Ð?è½"?Êí­ƒ4 Ð?ÔbAÎёŸ?Ôj¸ˆÕ^?åÎß—70?Ôj¸ˆÕ^?ÖP™æªÀf?·Fø>?ä׳ªŸÍ?·Fø>?ÎÈÁ«Ý_!?·¾ª€Ï?èMϕ¨8?·¾ª€Ï4FGL J1858.1-1821¿º¢L‹êÆ<À#]FÞ	5À;¯¥t™/À<)ñTk'@ v‡¬‡2@
 >ÏH¨?ÌǺ.d—?–î$"æ°?Ð"g~>tZ?þ6ÍVWP?Õ_"¥Fv?ïÈ!‡¿¿èxpT%ò¿Ýùu3ܦ¿Ý¤çá%If¿åŽx¾­¥?AGNbcuNVSS J185806-182314?ïñ6¡T#ì?bš¿rñM?]'½W¸(B?bš¿rñG?ïíkN?'2‹€ä,8?bpñ"o±–?'2‹€ä,8?ïÎ+¸E7?{Ì	°T´?xê#¿]e?{Ì	°T¶?ï~³ Ç´ú?~2òÆôÜ?)›ç	`Á?~2òÆôÞ4FGL J1858.1+7318¿çØòr÷Ëð@9k©Ÿ¡—À:qt4…BÊÀ<{Tç4@ôœDCѼ@…w£¥Œ?²{"O…y¿¶lþ[EB@E–È.›@_ûé
¿áˆØÖ+¿ãMMüUy¿íMÖýÓ*	¿ÁÔüÇuC¿Ú{"BšY¿èê–o AGNbcu3FGL J1857.9+7319GALEXASC J185820.26+731714.3?ïy!¥Ù¨?1"Œýg?ÛÞëDÊÙ?1"Œýg?ïO
ÁñuW?¶Ï".à›Ñ?–§ÁÑU?¶Ï".à›Ñ?í¼?⎖?¢ÓÜj8?²ëŒM?¢ÓÜj8?ï^E"H.b?"TAضŠ?"7[¶ú3·?"TAض‰4FGL J1858.3-2511¿À/ÿãeÀ)6~À¨À9!áKßÒcÀ;§5Þ^s@ÈWC"?@µ»8OÓ?±¸põ5¡¢?ÉX"*ø&@e8}@6sšœ³?ïü··ïÆ¿ßÞT~ÝU±¿åN¾Ôçx¿ä!H2ž¹¿êª¡Ô¦‹¿ïÿCAž0AGNbcu3FGL J1858.4-2509PMN J1858-2511?í¤CºŽ9q?¸}Gâ \0?²Ýâ+Ž4w?¸}Gâ \0?ïÞà£/T?''¾ƒÆü?p®hvÖ¸?''¾ƒÆû?èÿŠ"ùÝ?³·•‰x™?ÌÕ° ‹?³·•‰x™?î‡_­ø?Šw)1ØÚÇ?§Š ~>?Šw)1ØÚÈ4FGL J1858.3+4321¿×"z¨jJ@1>ž¡À:±Ðz×6³À<‡©qÛ@…z±!@›¹!]¹?ºH¦7Û?±¦ÿ!¢€ã?ïÁŠ¿66H@Ö%f
?í}Zi"?АC¯'9+¿èqÿ¡¶I¿ÛÔS±Wü¿ã€§û\,Q¿ïÿÿÊPËAGNbllNVSS J185813+432452?ïÜßų±?pÿÜpâ—{?q&{§@?pÿÜpâ—}?ïÒ.Õ>ÿ?‹fB_…s¸?vè•`€w'?‹fB_…s¶?ï¼rÛÐód?|SËàÃñ?€ãIÃ&Ô?|SËàÃã?îÌ}ýËÛ?ŠLT
NK?£8 .cB>?ŠLT
NK4FGL J1858.5+0640¿Ù…ìEè¼Ñ?÷øZðŸÀ9›=EÀ:…õ|ï>è@ ºu\M‰@F49Ãp-?Àå13ûÛ¿EłVž@[?çK©!?Çæ{Ÿˆœ?înÊî¦;i¿ì.KlåÜ¿å
ÃþGB¿áqüfîK£¿á®M?ùÀ AGNbcuNVSS J185831+064016?ÔonâÂ¥'?ÏE5ÆÞÔ¤?åÈHŽž­6?ÏE5ÆÞÔ¤?뱝ÌcGà?Ͻûðg¹?Á9ˆÎrà'?Ͻûðg¹?ãù-4ԉ'?¿ß²{@õ?Ø
¥–Vìá?¿ß²{@÷?ퟃr60v?¢k'ÿÂC?³änN|N?¢k'ÿÂC4FGL J1858.7+5708?è‰yL덪@5Ìÿ!³¯À:Æ÷–¤ò"À<¥¼ä!}(@ƒ¹ügÅ@ÉYø™Ú?DZ~è"Q×?ΫúÅ-œ@à f§ÔÆ@oüt°++?ïòæ§ieõ¿ÞF~1ß ¿âxP©e¿w¿Þµã¼¨gh¿ïñIï7Zà¿ìY? (ªAGNfsrq87GB 185759.9+570427?ï7	ã×€?œ[ R1åÁ?™Åïö?œ[ R1åÁ?ïr¦Ö‡?¶×‰€ë?œ±«%<Ï?¶×‰€ë?íëjâ€?£$C˜4í?·À¤¨ï"?£$C˜4í?îJÛÖ?"çÜȖA'?®¯K_'B}?"çÜȖA4FGL J1859.0+2329¿À™-òhy@!ÉdobÀ:M¼àÆ~ÕÀ;á<aNÏ@F×zzÅn@ã `ȗ´?Á,C܄¿€fX¤†Ý?À§H®ÅzÉ@Õ;@ráÊ?ïÿŸR@>´¿ßqªgG7¿èí5" ¼8¿à¨>b'D¶¿á¡HÌ!¬¿Ý¤ëGWAGNbcuNVSS J185857+233007?ïø|"©?wå@T(5>?~#øAî«î?wå@T(5:?ï㋖זg?Œ°Gò¨¿Ÿ?lti(i˜Ù?Œ°Gò¨¿ ?ï~¢îÖ?"OáUt?žþð+¢%#?"OáUt?鈴êïÌ?n*Ì"t;?†S¸EDÛ?n*Ì"t:4FGL J1901.7-5140?냗»{À6{þ;â
À;FÔánDÀ<µgÓMðN@nl <K
@è"úô'…?ÓÁi¢#?ãgþFÂ\@
0¡C§?ó ·?ïE´À¦Á¿×Ñ¡³CŽË¿Ñ¬ÿuìk¿äbÆÜ	¿íÇ4—ɶ¿ïó_2•AGNbcuPMN J1901-5138?ݯ'×`?Ì£‹ƒd?á|(>"wP?Ì£‹ƒd?ڙÏm
ßx?Ö½ŸÑ'ß?â³IzC?Ö½ŸÑ'ß?Ý	ˆMÓ?Àì«¼¯,?á{;Ù9t?Àì«¼¯,?«-ÖÁ¼Mz?"ü;³Åî[?îM""ä;*?"ü;³Åî[4FGL J1902.4-0629¿ïȨ¿ÛéÎÀ‡â`²È?À:Î-À,«ZÀ<sY"ð@!¬Ê†?ÿ4«ˆ¯fŠ?ÇSŠI{õ?@àWt7?˜4éÊßb@%'}?ÚµŠ;Þ§¿æ w~瑟¿ëB1}Ñg?§­?·T¿âøô=Te¿Ñ¸#@¡ÜAGNbcuNVSS J190223-062850?ïü T&˜ê?=86]f'?>ý^Ë8°
?=86]f˜?ïýT«@Ë?OðõºP?5Z£õù´q?OðõºG?ïÑt' ·w?y†éN'?wE¶¯¤Dw?y†éN?ï݋˦Q?be>n?q:uš,×Î?be>i4FGL J1902.9-6748?àX¼S{j½À:$咖pÀ8ðÜùjº‰À;ù$(Ô4 @¥Tƒ™@¿æ4|ß?¦O§!wþ?ÀǃwCXo@*Y:-ù8@‡)ÜÈBy?¯åµüÑ¢J¿à›NÛ/f¿ç')oe©¿è.¨>Íñ¿æHp¡þ—ö¿ïÿÿ^ðP`AGNfsrq3FGL J1902.9-6745PMN J1903-6749?ïþ8`\òä?,D~ ü0Ô?,yú0Ѹ"?,D~ ü13?ïú†#¤c¾?``Öûöÿ.?Eçqnqø?``Öûöÿ+?ﯥ¯yF?"Nï\;Ä?""!®y9?"Nï\;Æ?ïû¨I¯÷y?1ÐFìÎs?A^Ù@"ú?1ÐFìÎ|4FGL J1903.2+5540¿ÚrKþÂcR@4ˆäC‹À7òË/=ÛÀ;oáÔï@gÙØù×?ý+¡nz1?™(Aà ü?µpþÅÃC6@RP.ì|•@öfÏÿ?ïý& Ñì¿×«$˜Æ5¿Ü#Q©ß¿ÜK3o™¿âê+íĔ¿ã…]7»ÄAGNbll3FGL J1903.2+5541TXS 1902+556?©–¡<?"}–|Ò
?‡•šW°¥?"}–|Ò
?í9÷SÈþ?Äö–õ¿3?¶0Ea¼?Äö–õ¿3?ï8ºš<–€?–]ŠÎ)ho?˜è¬¸m0!?–]ŠÎ)hm?éȉÌþ«¨?«(Éxº–?ÈÝØÌQ`?«(Éxº–4FGL J1904.1+3627¿ÏÍÊ[B"[@*¾°1‹"GÀ9ê7iDÀ<4†6††@ ÔW§†Â'?üdÓSϊí?µÒ
_š~?±õoÙ+ÕÇ?û£¥Üû(@³†;B÷!?î[?î¿ìêg‡?âú°4撿Ûsµ"[ÄÍ¿Ûk:v"¿âQ¼‹6)ˆAGNbll3FGL J1904.5+3627MG2 J190411+3627?ïþ¬Õ¥c_?|¢%¹‹±?%2¥©ÊÝ?|¢%¹‹b?ïûq‹š
?VRiÖ½?B;åїÒ6?VRiÖÃ?ïò Ê¡c?kW^àd9?[¿Ìj½;Ü?kW^àd1?ïð«•Qœ?M]¶º+I?_¨Õ\Ê2?M]¶º+U4FGL J1906.7+5419¿ïõëf]š@3œ¯¢ðZqÀ;"§z¡‡À<Ò.d—YM@×3ÞLQ?þy™aܔ?Ðý'üft?à'`ç÷K@M;å‰\5@ºÂá¼s
¿äžðP_"ä¿áûR'L¿Ö#º"ˬ;¿áÁI̽¿ïÿÿ)@k*?Ì=Å]l¡AGNbcuTXS 1905+542?íI
rTê[?¶ZyÏþ/?µ·"mX­*?¶ZyÏþ0?í™í‰Ö?Å)Ô
Œþ?·K7à"±P?Å)Ô
Œþ?ãì‰ ´‹Š?»‰'¹Ý^ß?Ø&í¾–èì?»‰'¹Ý^ß?ìøs;8.?¢|û_n&?¸?f&>š?¢|û_n&4FGL J1907.2+0126¿º+Tbþ7ÀãªÿójÆÀ9Ûe˜áöÀ;r^‡tÔ@ lû™¾Øm@WhY…­T?Àè%ü¾Ø?ìá~à†?цW2üÂ@ uT•Ùq?ïÆÏ\Êr¿ê0¿»lR¿ÛåÞs=d¿äC¸§Ò¿ê¡É´˜c?¨y?ÜäÇëAGNbcu2MASS J19071198+0127091?ï¸:_ð©'?…hC×p?ñh՜?…hC×p
?ïý–üØÑ9?V?mËú;?3H9v9g?V?mËú<?îx?ÆN«k?œÒÖ'Øi?¨|›IW?œÒÖ'Øl?ïÆø±ÈlÉ?k
´,¹5S?|ƒ§ɛÀ?k
´,¹5S4FGL J1907.7-1232¿©dtê
ÎÀ"'ãâ"À:|Á>úÓÀ;Ç0ÄÃéÏ@róÜ[50@e*ýÌ=?ÌBÀÄÖ´?°Ïѹñ}Ü?坸ýâïN@4"û§Öž¿ïþ{€©Þ‹?ïø¼©¹L¿èŽÚù¶9ã¿ãlžä²¿å¼ôýîWâ¿äo åRÖAGNbcuNVSS J190748-123221?ïÑuÛJä·?wã«©¥c'?wEZ¤?wã«©¥c&?ïÍÙ÷¾W?":Qåç÷O?y ÔÓ?":Qåç÷O?íï‰ø5Þk?¢‡gÄQ³?°ƒ°>Qª?¢‡gÄQ²?ïdé|êp?'µPf†áâ?"bÐb±ÿn?'µPf†áá4FGL J1909.5+3511¿ê:ME¼*ã@'µI@»±òÀ;s•ûg¿À<«a«Ã@"•M.²?üzi¾	»k?Ðmµe'!,?²uÄ'aÿ?åP¾ÉÔÊÈ@óß+ôûj¿êwÄ?ì"Ô}›6¿½Mߢú¿°£ýöjœ¿èžHUh?ÐV±Ý³$AGNbcuTXS 1907+350?ïþ3÷8¿Õ?4]K¾2*Î?,ÀŒt§M?4]K¾2*Ô?ïý<¶B"?W7£ Y?7.Më]?W7£ S?ïÆۑÙO!?'ϗ‹!E?|'7XoO?'ϗ‹!@?ïó;Æù<%?PtÖvÓ¼?Yˆr
‡±‹?PtÖvÓÁ4FGL J1909.7-2140¿ìû%£Qå˜À+BªŸ{À:1"qê('À<O σ`@O'`Âãj@@×¾˜V£?ÄÏr™z?º=‹ÀÔ›?ôîÊ2¾™-@Àö†""ù¿ïÿæ4|ßO?ïÿ=ba(¿ä¼N/7ûð¿äŒ–ç7²¿ÜM Å¿ïÿwåëoAGNbcuTXS 1906-217?ïñh¼/ÆN?_×x{>`m?].‡ se¹?_×x{>`h?ï÷Wp#âŸ?pŠ
±™Œq?QQ¸:Ã*?pŠ
±™Œn?îÿÕ¡÷
í?–óÔqú[? ¥à!)?–óÔqú\?ïŽ)/ê{?}9ËâÏsâ?Œuœ4aF?}9ËâÏsâ4FGL J1910.0-2453?îžè܈ÃÀ-Ø$xGÀ:Š'Úb·…À<+¼•G$'@Zx¥-K"@sf³"@?Í¡¢§ŠH?ÐÂ÷+c±@€Xeã‹@©‡‰Ìœü?íÏ~x¿äò]®î?«ªÞU؜¿éRKý."h¿î±†Àyt¿á"Év7AGNbcuPMN J1910-2448?ïzgýz?¢ÿWÙ¹Å?žð³ Pî?¢ÿWÙ¹Å?ïÍPÝä÷Y?•šã¦Ë'?yW'
"S?•šã¦Ë?ë¹=9·?§Q]ÁŸÓ?Áõ½"?§Q]ÁŸÓ?î'Dž?'>¤Æ,«£?¦ë¿vÿE?'>¤Æ,«£4FGL J1911.2-2006¿Ø­PôŌÀ*v±=û
RÀ7΋8§À;<18‡0@}ædÌ@×Å>c?ž_ßÛê™^?ŦZݜ'é@$±Ë«d9@´œïd|V¿Ì8Lw§×J¿áÎÕ»ˆ×ª¿æ<tZDïô¿ç{tëdg‰¿êÿ`Ónu¿ïþê šª;AGNfsrq3FGL J1911.2-2006PKS B1908-201?îì‹QøÔ?¢ë(žÜC?¡7Jàr¾ê?¢ë(žÜC?îÓ:➨h?»'¾¾ßä?¢ÌQÖy?»'¾¾ßä?ì-žšdè-?®ö)¦5?¾",ؾŠ?®ö)¦5?ë¹ãúCÌö?²AÉÔjÌ?ÁpðÌ&?²AÉÔjÌ4FGL J1911.4-1908?à(PüÀ)Ä£çÑ5À9²×'2tÇÀ<"†4b@ ÁÀÓg?ýªbªCž?¶ã´3gÈ?¢îbÁýL?î,ný@	-ÆJ|¦¿îÝ2K¬§?ïÕdž½Ê¿Þ¶BFÌm+¿ÚNï;â"D¿Ù˜j¥:a¦¿ß'%¡ûAGNbll3FGL J1911.4-1908PMN J1911-1908?ïþRחc?#~¯‹¥ß'?*҆‰ÎE?#~¯‹¥ß¯?ïûÁ_¾?qJ&5¨Y?C´úƒýd?qJ&5¨Y?ïìßÈFÉ?gXùÀfã,?c 7¹r7¶?gXùÀfãA?ïî-½‡D1?Užå€?aÒBx»Íµ?Užåq4FGL J1911.5+0311?íÔ[G¶þÀ-<ÿdύÀ:¨ÕâDiÀ<"y™I@!–YÉË?þ,\\×q?эM{2ü,?ÜÄÑ¢@
Ö0'?ûóHàn•¿çzá³
Þæ¿ïÿØÝý Ó?ïýÖ$dcW¿Òç*{Ԍµ¿Ùi>›A:¿ïŽÎd|[AGNbcu3FGL J1911.7+03072MASS J19113134+0311093?î L3ºµj?¤¸Hæb!?¥û<ÄT©Z?¤¸Hæb!?ê`S›OVº?л†Øº?Æ~±'Â¥?л†Øº?ê"…ŽÇv'?°VÌîl-?ÇuéÄâ%º?°VÌîl-?ä!š¾‹
?ÂEôX
?׼˂éæ?ÂEôX
4FGL J1912.0+1612?ê–¥"§å@¿2/'À9ê#'¬?À;3³ÍêÚ@Ùà†"@u±ã<zÛ?Òl¸þæ?ÄÕÄÞõ?ñ'þKÊÙ®@<~€¹xÝ?ÒåÇ5樂ë¿ãåî¿â{G¿1X¾¿ärà цƿè‹6"çƒ1¿è	㮐¡£AGNbcu2FGL J1912.0+1609IVS B1909+161?ïË'ÒÌp?' pí§Èµ?KLä?' pí§È¶?ïú¿*S?m	q¥/¡?DõV·Ï?m	q¥/¨?힒A(¾û?¤Bžœ¡Ö?³möº(?¤Bžœ¡Ö?ïô…Reƒ?DÓk¦*â?Võ[4ùü`?DÓk¦*ù4FGL J1912.1-0803¿ï@T.†óéÀ zµ^ñýßÀ8¬™p~îÀ;~^sRÞ@ƹ†sø@"òü~¹?­‰w¸sN?¯wûd9æV?ÿ–xbm@ËN¢$'–?ï.rýMž¿à$åýö:"¿ä—‹')»e¿ã½/
/¿è1ÞõCd¿å',)S¶`AGNbcu3FGL J1912.0-0804PMN J1912-0804?ïøÛ7v<¹?L'l€˜ý?L""'
­?L'l€™?ïûá7
qƒ?Y)HŸBJÏ?@{#Ê9ô?Y)HŸBJÄ?ï•@¶ña?†sšßNè?Š¯üÒC§£?†sšßNæ?ïõ­¸@)Ú?FÏßí ?T¤¬I?FÏßí¡4FGL J1912.4-1222?âuš
[|ÕÀ$n9'ÈÅÀ9PŒAÀ;M¤Ú?|@'ñb~Š@®³Ý¾?¸×4ÀãÓ?ÌÎü|è³Þ@]žvx,@à'i¤‰b?찔[p¿×"¼uf´j¿ã"Àíp†¿çs¢¡¿çG8¤¿ïÿôA…ÜMAGNbcu3FGL J1912.6-1223TXS 1909-124?í؃¨b~?¶
tiKo?·á;â¼ì?¶
tiKp?îöœÊä?·r`Þ¬Ì? ŸÖ6óQ­?·r`Þ¬Ë?ç>\ñ] L?´¶ÜÞÙè?уFD¿g?´¶ÜÞÙè?í¶ì"K5?˜£%ø?·ŠH›Ý¦V?˜£%÷4FGL J1912.4+3738?ïÿû샖°@(´¡ß¹8›À:š.$ÖyÀ<CLu#˜‹@›C×ñ1@LG䛬?Å´'åLJ†?·Þh«?ûU_]]©)?ÿ|Øm¿Ì?ïîõ üпâcåîy¿éûP£†'f¿ÞáÉÿ={¿ïÿ~›'?ïõ!¬ˆŠAGNfsrqTXS 1910+375?ïC[Ÿ¾§?°ƒ$#Wȑ?—"Œ+ ?°ƒ$#Wȑ?êt³†ÊÓ?͔°P`ݝ?Ǫ-1äÔ²?͔°P`ݝ?î«:Õ3#	?™ì©

º?¥LR¬ÍÏw?™ì©

·?í1«ê=U?£lqí'Àæ?¶w¢ ®Z?£lqí'Àæ4FGL J1912.7-1250?˓vò%Ë^À$ú#9ÀëîÀ:&êÏS)À;ÑÛ¤$é@ 
¿)öôi@BZƒU?ľªŠ­˜?±5ä¾[?ðãœ*Ù@oL¶çÞ ¿ïæó{??ïzOßK¿ådÂÝ_¿áà³~È¿äxgêŒÑ¿è…2ˆKAGNbcu1RXS J191251.7-124929?ïë+ 5ÖT?f³ËàÕ?dÔ_Ê)«-?f³ËàÕ?ïùÍ¢{'Œ?dбòìî?HÉv¹Öý?dбòìò?ïkh¯o<'?›Tª å?''êmŒ?›Tª å?ï•ìtÜÊô?|fi‰ò1?Š"âÈÍB‰?|fi‰ò.4FGL J1913.0-8009?ïŸX?À;žêúµ=dÀ8ãÜEԉÀ;·%;ù«R@yiÓ®=k@±ƒÞFqÔ?«Îªžœ8?ÂWzzÅn	@§Òª\_@:Ë-?€{¶@ˆ¿ßÓ þ½¶¿åìÉ⌧™¿æáìï'{¿ê{÷"J¿ïÿrÁ¾{ÑAGNfsrq3FGL J1912.9-8008PKS 1903-80?ïöîË0Ð?NÝr¸4G?R"iûža?NÝr¸4I?ïùœAšöF?aåU­á?IŽù"&è?aåU­à?ï‡ÏÔ'p?‰ô'š25?Ž
ö>$1?‰ô'š2??ïû5Ž¬À{?5XwJ¯®?C)ÅLþ?5XwJ¯­ù4FGL J1913.2+0512¿æ™5‰.¸ÀÊ›š$ÚÀ98
¢pÀ:ÕÈ­ç.@ÀŒL©ý@úo?Rü&?Êj»ìÕ¬?Ë­G`ç¡d@¥s!_Ì@KÿßÝ6?ïJ|€Y+À¿áU)' ¿éøn¦¦ÈV¿æ¼o»¿êě¥ãSø¿ïÿI)>¾AGNbcuTXS 1910+052?Õ¸·›©?Ê	ÙÇÒW??å#¤2~+1?Ê	ÙÇÒW??åDUÔ`_ž?ÑöO€—ê¥?ÕwTW?@Ã?ÑöO€—ê¥?ÝMý¤£?¹ø%¼Ö!?áY-ý±/?¹ø%¼Ö!?ÚÁ—'kçÎ?´fÓól‹?âŸ46Ê?´fÓól‹4FGL J1913.4-3629?ÔðýsvÜÉÀ3ÚªŸ{ZêÀ9³æ鮄ãÀ;'ŸJ³'@ë€nÐBM@$FE^¯?»ßð¯š?ÅÀüI'I@ˆ=ÿ?à@4¥/úĂ?Ѫƒ ÜD¿ä"²ªØ¿Ødñ†Ày¿ä'Ù‹÷ð¿èÈòýãñ¿êy
By!TAGNbcu3FGL J1913.5-3631PMN J1913-3630?îïYŸkø;?œ4'¦\à¾?¡
f	@|B?œ4'¦\à¾?ïúi@`ΰ?`Ù¤[7à?FZþ|Å?¯?`Ù¤[7Õ?ìò>ܛÎs?¥¼Eànä¶?¸n	!Œ^?¥¼Eànä·?ï°ÐÞ3ý?q4£^+û?ƒËÈs;Á?q4£^+ü4FGL J1913.9+4439?í;´î¨R£@-ó*k
•À:I¤¿g‰|À<t'Ç=@Ó@£%2g±?ÿJ£ý ª/?ºK_ú¼t?©æª!.×b?ðs
=Ö$@*fÅû?ïö Kºi¿éï=n¿ÒeÎÜŸC¿Ù÷½j.G¿ãV½¢…¿çT‰Y°u~AGNbll3FGL J1913.9+44412MASS J19140184+4438323?ïý(iû3?30yP?7Þ¼°&h)?30y%?ïùàAt…?cm!A`n'?Kø~ú-ëJ?cm!A`n†?ïí¦4«#?q1†Æ?bYËbTÝ]?q1†È?ïµÏÜoÜK?jòtÿ¼U?'ŒäíJ?jòtÿ¼P4FGL J1915.3+1149¿âï¾û?ö}*"=mÀ8vW0h}˜À:º|h0@љÅäPL@k9ýQÏÖ?Ã`qšL
?ÖFíD'o@¸0]•Ý@™Õ­œ¿ÔµŸ^ª…O?éO/]e¶¾¿æ	!ay—œ¿èy‰Ž‰›¿ïþ›{ñèæ¿ã¥ÁX¨8AGNbcuTXS 1913+115?m¨ç¸/"ë?'ˆÍäÔ?ïâWGÐÞ?'ˆÍäÕ?{Ö>ÂÂöC?ƒ}™l—ˆ?ïÈS'zz?ƒ}™l—ˆ?ŸëRÂ8Ñõ?•´´bZ?ï¥iî9q?•´´bZ…?jÔWŠËÅÏ?ZGèÎ$´?ïå+¨u4<?ZGèÎ$´4FGL J1916.7-1516¿ï÷ØÒ·ªïÀ(Èõ\)À9ÌѝìåqÀ;ÄSõJšX@#>¥ØW@oúcÞÍ?Ãû×ý,'?Ðô!ºåĕ@ð@|ÇÑ»@D]ÓG?ï¶A……¿áøŽâ[X¿éƒ†="	¿èTÒõ۹пë¨"HK¿ïû÷"IôAGNbcuPMN J1916-1519?‰—?š——î"ý«?‡¸`3?š——î"ýª?ïõ7/u–W?vý‡­@f?U'¡ÓP¥?vý‡­@j?ì,袘ó¸?¦èÞÿöã"?¾˜ºë8bG?¦èÞÿöã—?ïÃt¬çƒ?jx{³\$Î?~E©Œ>?jx{³\$½4FGL J1917.7-6442¿"•/­þâ¯À;•»¾‡À;	ÏDvQ–À<ªJaÎ@÷\"ë'`@œ2?Ñãâ» ¨?ÕP–ñH­@=p£×
=@'ŽÇ®Û¿ïÿÇ*Ì\e?ïþΈ°=¿á%Óύd¿çòùℚ¿ßë,~Ž%r¿ï¿ü¥¬¨AGNbcuPMN J1917-6435?ïÞÞüø{Ö?r<ع'?pƒÂë?r<ع'?ïîÃóÜÌÇ?zhp»,ôÉ?a<#38Â?zhp»,ôÈ?íêCÏL??¡7Zî͔É?°­á…ž^?¡7Zî͔É?ïBœœ'Ý5?…öZW?—¬lo¤YI?…öZX4FGL J1917.7-1921?ê.Ü2àalÀ,¥(IË%-À7õ"i†¬WÀ;jUõÕÛ@âÈހ©^?þšÈ:£j?šlûÅ¢zØ?˜\ÄÙ?üp'|F¢@:ŒÁnö?à­ÆÂqª¿Ò‰½#ã4¿à_Ðéſ۞üd¿ó ¿á5Мe&¿×èÔjOÿóAGNbll3FGL J1917.7-19211H 1914-194?ïüݥã?61Â܌¡ö?9ëyÐì€?61Â܌¢?ïûß|×q?eß^w(Ø?CĂ¢<[?eß^w(Ù?ï˼dыx?ƒ¹¡¦kàj?z!͗:C[?ƒ¹¡¦kàg?ïìÏ$cN>?V—7æz·à?c0ۜ±Á‹?V—7æz·Ø4FGL J1917.7-6930?è ²Õ坫À;' hUSïÀ:NãF¶žÀ<p(ßó@Òë1¼»ˆ@SX"?½qõ:Õ?'Ç]~4Ê?Ô$ þè¨Ë@
0#	ÅP­?¡UMºHä¿ÛIÞ}¿äzï,D¿æ8}¿H€¿ãÈM Å¿Ñ×DÔñ4AGNbcuPMN J1916-6928?ïüéû/þ?3b—ì$>?;€°&€
@?3b—ì$P?ïþٙgå?A£lX'"?#Æfi¥k?A£lX'–?ïâæízà?ni›Sm}?m…ç!Ë?ni›Smk?ïþ±Í§ïD?ف.W?$ã%ĸ?ف.G4FGL J1918.1+3752?艊^"+'@&à=ݱ ŸÀ:Â7n+VÆÀ<vÒõÛ¹Ð@ |ú<ü¶?þÓCßRáN?Åb}äzC?¿H‡h:&?ùf'•ù@sBdÔjü?ïùfˆË?ï³!å#¿Ð_¾+Ÿ@¿Ý0¥dSÉ¿äD-÷Š¹¿ÝfN=¥§ðAGNbcu3FGL J1918.0+37501RXS J191810.2+375315?ïûa"ܳ½?AŒuËÎÏ6?B{t18?AŒuËÎÏ*?ïòˆÃæ¢Ò?xˆào‡â?Zîx2º[Þ?xˆào‡á?ïêr{2Æ?mÃiGˆÿ:?eb"Í:|?mÃiGˆÿA?ï«r©¡uì?sˆ;È5‰?…#U—¢"ñ?sˆ;È5Š4FGL J1918.2-4111?Ê£ý:ÜÀ6=cEI¶,À8^&åGÀ;wF'‹ˆ_@3,éŠ?üíy¾Ô?¢ð"½DC§?»œÝø©Ê@ãÔHµ{@ó8–õOx?±
9>æ¿Ø6êx´G¿Ú
Jk^ì¿ÙÖØ9¦ë¿äw^o¿ç;C£AGNbll3FGL J1918.2-4110PMN J1918-4111?ï̔MVå•?€zëÏÍeM?yµÙT5K?€zëÏÍeN?ï´J§¨¿?–Žéc¾·?'íOVÐk?–Žéc¾·?ï_p¡vËÙ?"FÿGJ`?"ëÑ&"Â?"FÿGJ]?íùvÌÖ?"e*srbý?°4I™OgP?"e*srbþ4FGL J1919.2+0618¿ä)Þ}w8À
!ÇÃx5À9wEšMôÀ:ö@&t@õøADÃÔ@ïOP ?Ù*æÞpä?ߋ:[E ô@	áZùJÚ@ÉIýúí¿Øí‡Â׀…¿àâeàÚuØ¿ê"¦žô:¿ïÿÚv»œ?ïøÍaO—¿Ï€™XG#AGNbcuLQAC 289+006?ä$Âd¹}œ?ÏþÞD€
?׶{6Æ?ÏþÞD€
?C_??¿è²+}Ô8?¤¯Ê?¿è²+}Ô8?Þm§UAi?½í+€?àÉ,U_pË?½í+?ï!&¹Þ?œƒvW>?›Û(ÝD9?œƒvW>4FGL J1921.3-1231?ï«ã··À(|Ä&5ïÀ9þ‹‹¹ÝÀ;ÙQAK$@ìÀÜ©Ž¯@$'ÇÅ&?°€m"Ã#?°ö AÏ@0
ø'@ªÅÎÖ½?çÏó"
3`¿Ðÿˆá»q[¿âA:û¿Þžœ)¥ì¿á¿ï~Óo©¿äҌ)nŽSAGNbll3FGL J1921.2-1232TXS 1918-126?ïêiæûA?e"ÔI†	8?e–¾å?e"ÔI†	;?ï¹ÿ¦¶nM?—Ò±–.ê?€Rdlƒ?—Ò±–.ê?ïF‰í¢ø?Šlý˜ÚÔ?ˆ®]"—Bw?Šlý˜ÚÔ?î>'"02<?"½8˜o?¬ÖÌüÜF?"½8˜n4FGL J1921.7+5817?¦,Xn#ë@3	‡¤¤—À;Ãú%Ëk¤À<õçoæAé@!×Û[/ür?ú}$ƒmj?ÐÃqnØ$ð?¼Óæ``º?ñ§Sçáv@öh@†-?ïÿÍ?¹Ss¿ïÿ'ÌÎzL?ïÿ°ï÷t@¿æ#Ã>-¸¿¹øk µW:¿áG»ëÓùAGNbcuWISEA J192158.68+581708.5?ïÿ…¯hA4?þO"0•é?"%ï³p?þO"0–›?ïù6fxíb?f³;â³?K&fJ~û?f³;â³?ïÔ	Þ'?y¥f‹A?uþ{þ6Ô?y¥f‹B?ïãj˜ù´?dèx¢]›#?lú•gK€?dèx¢]›"4FGL J1921.8-1607¿îšŸÅáå'À+¾¯«SÖAÀ9NjXŠÜÀ;¹ðál—@ )`^dL?û;=Žc?²c/¾ù>_?·m?Énžn@Ѭ€&+
@
ïß´tç?6ä•¿£Ó=@§¿ØÕD€ª³¿Ð*b{ö¿áa'Ú¿×IÅEïÎZAGNbll3FGL J1921.9-1607PMN J1921-1607?ïýq×ò#ý?0#îÕï#Y?4q@nà#u?0#îÕï#‹?ïú.]œBû?\k>%?GF‰Žô?\k>+?ïÒþúlí?y›JaÞØU?v€'ɉ8€?y›JaÞØV?ïâ4'Ž¢?XžL?ÂÇØ?mæËØq^?XžL?ÂÇÏ4FGL J1922.2+2314?ì2~ZB@!0¾
í)À9Ò°@¥¾À;¶_ !¸@ ˆaV݁@x˜:	?Â^´Á=L'?½Zž\! ?ýEª~Ä+>@âw¯äà¿ï²xË'u?ïüá½tÀ¿á8&êþ¿ÛT÷=¹žó¿æUF˜¶›¿àjëø?AGNbcu3FGL J1922.2+2313MG2 J192213+2317?ïLJºÀt?ƒ¾Î³þäº?|<"üŸÅ ?ƒ¾Î³þäº?ïAV?&M¤?¨9k£Ž'P?—Õ86K£?¨9k£Ž'Q?ïsÅ~¸?›è±¿ÄW:?Ÿ±žçP(ù?›è±¿ÄW9?î
KÚ9ß?ŸNŽ쿓?¯+B\b"?ŸNŽ쿔4FGL J1922.5-7453?ìoD'ë²ËÀ<#ædM‡À:Õçþ{À<fH;Øô"@ Xr…®€?ýA"d~.Ú?½î^Aÿª?°!a#±`
?ógû&|k‹@	™Ñ;Ü?æ|
A±ü¿ã¶Ã«»Û
¿â2§Ý!ž¿ÐJoD³8¿ãâ"i·S¿¿Õa8¿!œAGNbcu3FGL J1923.2-74521RXS J192244.1-74541?ïÿÂ<Ê?l M;?§¸f¿Û ?l M;@?ïþ'T#,å?Cz訤¤?&Ú½Í1œ¯?Cz訤¬?ïúÍ0øD?HçB	â ?DË<¾ì3?HçB	âÑ?ïõ˜Ê±rÅ?D8è5|g?TÎjw?D8è5|j4FGL J1923.4-2503?çÉœ4gÀ1ÄþG™ÅÀ;w/âEÛÀ<£|§‹@"RßÛGcí?Ø©Ý3¢D?ô[D)$¼?ïÖų,é@X> N¿@`̇­ˆå¿æ¿ŽU˜¸É?ï"Fj^¿á/ÿ¢/?ɅsFô†$?Ætð'^"‹¿é0…;=ÄAGNbcu1RXS J192325.9-250228?ï»"Á¿"-?Y+ö¶J?7Oôg?Y+ö¶E?ïùùÞ5'º?fõ²ëŒ+?H‡)µÀ?fõ²ëŒ+?ï=ˆàÝ?˜ízüÅS?øNNãäD?˜ízüÅQ?ï÷äDK?V«(yǝ?QÊ7Ñwk$?V«(yǖ4FGL J1923.5-2104¿¹8P"Ž4À0>îؐOnÀ8¡Ïi_?+À;¨''ûÈc@øÄI¦@	<Ú{áù?¥òÀ§Oµ?ÁÒw[¬#4@ù&âÂØW@0—d54?œ!¿Ýø¢¹ì¿ã×Tæb¿ãÓ?ãDÞV¿êüí@àšà¿ê«hÎör¹AGNfsrq3FGL J1923.5-2104TXS 1920-211?ï³RQ
?~½ý™M?ƒ:+|+¼¨?~½ý™J?ïùi¿Á?`Hvõ²Ëª?K¾YûŽc?`Hvõ²Ë°?ížé× ó?¢‰"ü¹î0?³±Føg ?¢‰"ü¹î0?ïÿ¬)ö>ý¤)ÞZe"?õ'{xW4>ý¤)ÞZb×4FGL J1924.2-1549¿ïï"çÀ,†)Ø@žVÀ:õ™ÊARÀ<EÏ¢j"´@ È¿èbÕb@`b
·'?țëƒq9(?—;ƒ8Ú.?Ó ™?׆@k¨÷/¡Ù?ïµ;K/©;¿ì'Ë $c?ÞQmü÷¿ê7‰Úõ¿œÚ»ç'
¿àõ¶€Z-sAGNbcuTXS 1921-159?ïýóˆÖ?2ɐœ&Aî?3hc¹N4?2ɐœ&AÈ?ïþüi"_?:fÄãl»›? 9nVÊh?:fÄãl»ä?ïÌ|¬³­?|ú0nX;?yÁ©¦)8i?|ú0nX<?ïõ1¼w<F?LꧪžSa?Uœ‡‡xg?LꧪžSu4FGL J1924.3-5458¿ïáÔ¤¶EëÀ:"œT]À;OÖNUÎÀ<Ãü7ôc@ I£ÿyw?äԌê^®?Ú|"zÔ1›?‡ça@9ÞýPù@'²¶v??àbñNŒU¿×AV¨¿ê\vXKñp?ևáá1à¿èâ¬K¿ïþ Eð¥AGNbcuPMN J1924-5457?ï˜vË(¶ò?‹Ô@±CSñ?‰âM5ÒCT?‹Ô@±CSð?ïÙm`½ÜÐ?š?m^{œ?sIO¡˜R?š?m^{?î'u['?™'2˜óµ?¦ÞßتM'?™'2˜ó´?€¼åì?‹Ð¾ôýp×?Ž_ÐƄ®?‹Ð¾ôýpØ4FGL J1924.8-2914¿ïâ]ô½	À3›ûz_A¯À8ªX-¾À;×/¸ToÄ@ú';‡@ò\f2d?¡¯Šœ¦"T? ¤!²Ø/?ø.8øo@‰ê¾ÒŽ¿À–—Ü€¿â‹…Û¿æþA¹Þ³¿ã8î~Mbß¿åÙv0¿ê$-ÁÚ*ƒAGNfsrq3FGL J1924.8-2914PKS B1921-293?ïýßox?*uå?1T"?'ë?*uåQ?ïý…­uq¬?StëTDh?3ҔTr–#?StëTDg?ïω(5?ánN£[?x;kåqúØ?ánN£T?ïÿµÅ|§>ú¤ÃIðDó?Ž Ö?fk>ú¤ÃIðFI4FGL J1925.0+2815?à-OJhÜS@AS½vdÀ9œIlÊ.À;þ)ÊÔ¥@ W)HΦ?ÿW¹Ëh?´øá.-»?¤ý"ãél?òÛHZ⤥@C ,pKm?ïÿ"å­nc¿Î‡ rÑ®´¿äOÉkï<¿ÔrÔ§7¿Üø°WK@¿âÁ6á¾vsAGNbcu3FGL J1924.9+2817NVSS J192502+281542?ïô¾¶F:W?Q­g
k*_?V'"s‹P|?Q­g
k*`?ïëf'­g?y¦¦—•w²?dã™nR˜í?y¦¦—•w°?ïÄm֌ö4?~¶¹~'I)?}ɹ"åë?~¶¹~'I0?ï/ûA5c?€HàƒùÜ?š€—ÙS¢?€HàƒùÜ4FGL J1925.1-3358¿¹™›ÚdÊÀ5H¹ý½/¡À:qè«O¥À<‡çÀn@Ôíè¦G'@ԏ¿%D]?Õmfr{?ÒãízÂ=þ@lû%¥«÷@•POù'~¿ÆIà‰B3¿ém2}«§c¿àê^u׿ïü?OQ¿Ï‹Å›€$¿ï©$Q ˆAGNfsrqPKS 1921-341?ïø*ì_#<?a'ô?OTNƒs5?a'ô?ïýƕ
÷€?IÈÇ뼘?1ËW¨CöÛ?IÈÇë¼"?íÞós•!?Ÿmù ËÌ?±dcW>ò?Ÿmù ËÇ?ïñ‰ÑÙzE?N'ìÖ¥D?\ì\Mt?N'ìÖ¥>4FGL J1925.1-1019¿åL5³?=À(@^_0çÿÀ9"¸:n×À;†¸›½`H@Ì®EM<@Ò<B¦m½?Á†Ë¡(¯!?½lvìÚ^@`GMœk@¯Ôà—"ì¿Ùû/€÷e?ílkûѝ¿Úö` Éd¿ã,'Ž2]J¿æ>o;÷ýÓ¿í0¯_Ô{îAGNbll1FGL J1925.1-1018PMN J1925-1018?쎴9š:Ú?½B
ŠÝp&?»Š^3.)7?½B
ŠÝp%?ê÷eÃt?ÊkÛ{°˜®?ÅÀ"hò/ð?ÊkÛ{°˜®?ì²X©^€Ô?ª>SKѦÙ?ºm:µùW?ª>SKѦÙ?å"ÙQÊnt?¶íöíj?ÔØM\k#?¶íöíj4FGL J1925.7+1227¿æs·8	ɺ¿ü†«pÀ9á²7QÀ:È[;ù@¸žÅÓ^a@§;ãÛÝ?¾TÂ(Y?ǸMú3ã1@ïƒæ©í¥@ë9Û׿ÁÙ}µ7"Ò¿á¡Î¡¹"Ì¿ãȑûž¿åªÆÇ©¿ê|=2v¿æÍÉ¡õÔAGNbcu3FGL J1925.7+1228TXS 1923+123?삚sÑèã?·\¶'UT?»ë,ap¸å?·\¶'UT?ïûCÁÍr?_˜7cÿAl?BðûèÊ0Z?_˜7cÿAr?çÇ:%±Ïy?³­{Z1Í?Ðq‹´œa?³­{Z1Í?ïޏßÛè"?aH/tÙºþ?p¸¾:?aH/tÙºþ4FGL J1925.8-2220¿ìlS^k}À1?´åOz'À;GoçïhÀ<ˆÇ:¼"p@"!ëu(?û¦Ô€u?ÎMoÊhC‹?³¹? Só?笇²çHy@'Eã-¿ïö^½|?ï±Oޏ—ã¿à]LÁú‹Í¿Âï,ÉÍ¿â¢y|¿ªYÆ<\I$AGNbllTXS 1922-224?ïÿN'ü?kór*‹?V/ }ÀÌ?kór*†?ïû ¥jlT?c"‹‹Æ?C}jVN®«?c"‹‹Â?ïò×.l¢?ZÃ/^†ëû?ZQ£&¼ž?ZÃ/^†ëö?ïàN|Qj·?cŸc¾#‰?o±ƒ®•H†?cŸc¾#‰š4FGL J1926.1+2059?Þ^줖Ý@v]¤öÄîÀ9†V›HÀ:÷¶‡æê@Ð"—¯Š@ž9ÛT?ǟ¬ƒ+C%?½Ùß‹?øB;ëh™?÷ž§ªÿH?î+h~nšè¿äIî*ëf¿æWð}ðÇ¿åâK^Τ¿ï°Ö+ñ'¿ïý,ÆAGNbllOV 239.7?éiŸ¢z»{?ûvSð
?ÊYv?ûvSð	?á'gôgRÂ?ÖEüL¯X}?ÜÛ01Z|?ÖEüL¯X}?èX>ycê?±µ#K?«—?ΟâpV?±µ#K?«—?Ïå]JØ÷?®ÜøË2–?軨­IÂ?®ÜøË2–4FGL J1926.8+6154?âý˜¸¿€@3¾š^»w:À9ñ\Ï
ðÀ;Îm=ðüW@Ã@7ü?üŒ•¿ðEx?¬« Ðg?µÜÃdïû@|XƒNÔy@>C">™C¿ã`䡪µ ¿¿öÔ]9ìá¿ÜðÄ£ÉH¿Ør/ÈD§Ð¿Ûwp#ÿc£¿ãZã±àbAGNbll3FGL J1926.8+615487GB 192614.4+614823?ïýÝa9¨Ø?+A$vF"K?1ö2¹G\?+A$vF".?ïôH™R¾Œ?pIŒÚTSb?WnÍZ'æ@?pIŒÚTSd?ïݺ³F££?tÁdQœvÅ?q"¦\®/
?tÁdQœvÅ?ïç@ҍ²œ?V4#rÆü‰?h¿-rMdë?V4#rÆü–4FGL J1927.5+6117?ª‹:x¦@3qí9SÞ¤À9d²<'ÎÀ;îQ°Ì¼@s7ævA%@ÞÄK?¬l«`&Âs?³"ÁO"ç@+
=²é@
¸`Ú
x?ï÷náàb¿Û&¢+8'ï¿á½< —¥#¿ã;©p¨¿ä{`H•¿â¢^d9eAGNbll3FGL J1927.7+6118S4 1926+61?ïõÊ9/Êý?MsL>˜®?Tk j?MsL>˜˜?ïïÀM—Äí?q"÷5¿*?`?²h;?q"÷5¿(?ïºâ6dñ¬?€ððWÚ	?GrfÔó?€ððWÚ	?µÜ¯?lˆàìy?ˆ\~'ˆÔV?lˆàì4FGL J1929.4+6146?â~rµ¸÷J@3gag#$ÈÀ:t+'~B%À<'z@¬Þoâf@$&5îþ?ώÜð±X?ÃÁ• ¹?úNêHޖ@}}¸'ƒ%?ë™.9Ï/¿ÝÖUa±Jæ¿èÚò)}¨¿Út°`Ûb¿íޥœÈ"¿ïÿ±@LAGNbllTXS 1928+616?ìŒß2Ö¤ÿ?·sð|º²€?»™iJØ
?·sð|º²€?é¹EšÛ®ë?͸hð;¿M?É锑DU?͸hð;¿M?ìÿÂ^÷¿?¦µ@UÖy4?¸íB
?¦µ@UÖy3?ê5ˆ»3n?¦ñºÍvsP?Ç)Ý2GŸ?¦ñºÍvsP4FGL J1930.3+0911¿™»¤LíFÀSÛ]‰HÀ9)êFZWdÀ;ñ`®—@qÇO_c¾@8þžÖð<?ʋ ÆÒ?ÕC!ór@Êôj ‡Ê@8ú0³&3¿ëœA^ïúy?îâþgy‹Ý¿ëyIbI¡4¿èÑ[§Æƒ¿ïû•!ººÑ¿Ö‹N<Îè[AGNbcuNVSS J193016+091037?â¸õB!D¤?Òd
læ!,?ڎ{½v»?Òd
læ!,?Û@ùöÛö	?Õø²	?â_ƒ'ý?Õø²?ێ܆/?¼[¾"ö?â8'¼è8r?¼[¾"ö›?Ȼҍ•?²ErG·Î?éÑxœšº?²ErG·Î4FGL J1931.1+0937¿Þ¸©‡ó?¤À0É°·À8=éˆÅ6À;2'î"­y@ ]ꟸ?ûfÙRí
?ª­NWPôº?¸OÂ5<g@Fß?–@ò…-H?è#qߖS¿çè| åhO¿×ùÎøö÷C¿Õ¿r¼`¿Ún?¿ÜaˆE´?7AGNbll3FGL J1931.1+0937RX J1931.1+0937?ïÿã"G?,€??#vþG?,´?ïúi")Ô?]Ï%Ñ??F[Á¯X´Ê?]Ï%Ñ?ˆ?ï?+uþ"L?–}κ›Kþ?˜'@;¶w?–}κ›Kü?ïâ´,Ý.?Z…Ë¡æ[ü?mKáÓ"Ф?Z…Ë¡æ[ò4FGL J1931.3-1556¿åV—'À/¾PÅë1<À;u–²^Œ}À<Ú.Íû¡@ "´+?û=\ÿµW?Ù6¬Ï×CH?ëpý
':@¹ÿ]BÑ6?ÿ¨C0¬E¿í"½«;X¿êº¬(©l?ïó€`°?¦°×½…uå¿íxa"·¿Õìò\(téAGNbcuPMN J1931-1558?ì^!†Gèµ?¸šlQ_?½óÍÀºP?¸šlQ_?ë@ïòEœ?ÎG–°›p|?ÂüAÀ6é"?ÎG–°›p|?éÏüæHLÂ?± iÂD\?ÈÀfÞÌö?± iÂD\?æîšg€£<?¿sÂ{Î¥?Ò"Ë0þ¹ˆ?¿sÂ{Î¥4FGL J1933.2-4539?á¡ÞÊ$ØWÀ:	¥e¶šÀ9Ð]ÿ—¸À<3Ð$ër@'.ϏÐ@Ïf"‹?·èÞü$SF?©¦>(ëÃ?íÀ‰þ#r@
ìª``ö¿Í…ÁµíbD¿å¬°Í'Åj¿ç³:¿ïn¸¿åíLŸ¿ì¬•à–¿ïúï,DAGNfsrq3FGL J1932.6-4537PKS 1929-457?ïýGõÚ?6ïêåúöÄ?7ÀQ/¾1?6ïêåúö¶?ïþô},£?;V¼'e†v? ¸-5Ç	?;V¼'e†/?ïê6é?fH~U¬¾?eɀùù}?fH~U¬¾!?ïùÁhÎ99?8÷Q_vŒ?Hú\Ç?8÷Q_vÏ4FGL J1933.3+0726?íxîݳZÀM;€ßŽpÀ9!UŠv(À;½=1¹¶p@ ß6<ýâD?ü`¬}¡ìN?±4è%ü¿?­M	âÆ£?þ(³}pn@ì{"`'?ïÿÄ;-Óx¿èkþ‹‹¹Ý¿Ú®(ýân¿ÔpŸÌä¿Þ¾"¯<C¿Ùyª	bAGNbll3FGL J1933.4+07271RXS J193320.3+072616?ïþàêj†f?"YÜÏ>Î7?!ñYW™Ÿì?"YÜÏ>ÎÙ?ï÷‡é,ó?m4Hádã?Pð-¦Ԙ?m4Hádê?ïÚ_i›Ãv?w"ÜHÖÀ?rÐK2E(?w"ÜHÖÇ?ïu7¢}Ûò?{r¿‡J,?'Y°Dº?{r¿‡J,4FGL J1933.9-1025¿ïüÃ}û'†À,;}æOUÀ:™Á•a%µÀ;¼,k˜Õ@VK˅yý@Û{Òv?»4‹"'Å¿º¦ƒŒçÚo@Aâ"Ÿ@†Õ/ò¶ì¿Í™—@MøÜ¿éoÜfÃË¿í—Ù¥ù#m¿Ö
‡­ÞÊü¿¥K鞥Ù)¿ïÿ•ÂûAGNbcuNVSS J193349-102530?ïó ƒ_?fƒú%͘w?Yð¾ù×?—?fƒú%͘r?ïôiº}ù?ƒ@LjšÙK?W,‹xÛ?ƒ@LjšÙI?îÊøƒI?™..ßá‹?£P~§Ëƒ?™..ßáŒ?ïí¿ÊTX?_&‡Òü¹ ?b@5«ç¦?_&‡Òü¹˜4FGL J1934.2+6002¿çøÐòœ@25Ôèû½À:ç|ò™åðÀ<«Þ7X\@ uҕ¹/?ýo"èbT‰?Á¾BuE|?ÍD<ÅÙ«@Ã$­^r?ù(ǬÒ['¿ï}'›x—?ïÿ˜k¥k?§ÿÚýMY`¿Þ)¡"I¦<¿å?4(%¸÷¿á9âyÝ;°AGNbcu3FGL J1934.2+6002GALEXASC J193419.64+600139.5?ï5ûœÒ5?–ѧçÜÜd?™@Œe¹^¡?–ѧçÜÜe?á›J'XÙ~?Ó¿z‹Œ"Œ?ÜÉjûNM?Ó¿z‹Œ"Œ?ëÕ"ñý{?°
ùMõ½x?Áø©°8
?°
ùMõ½x?Ýçó‰°}ý?´'Ãu
%?á;'Á?´'Ãu
$4FGL J1934.3-2419¿èÏmÍæÌÔÀ3Ìu_þmYÀ:¸£a™xÀ<psT‹r@!	L;P?ùiU~·–?Ë!Õþ#ÜÔ?Ò7A_ƺ@к%*\@U'•ñ‡¿ïÛ>ê÷Z??ïù> #Ìc?ãÇ¡A(¿¿ØáŸÂ¨†œ¿ãǂÀºí¿Ù‹n]«¬ÂAGNbcuNVSS J193412-241922?ïá…Ѫ?rÅÏr-?nýz.ÿT£?rÅÏr,?ïÙ¿nÀg?"džñmv?s HŸ¿L
?"džñmw?ï@ŸwhB?'Ë'Cµª?—ì'÷ß?'Ë'Cµª?îÑ°(б?ÀXY.Cò?¢äýrÿtì?ÀXY.Cô4FGL J1934.3+6541¿ïÿœF8¯@4RmzVÞ3À9ËÆ<ÓGÀ<J<Q†Û@ߝâ)@/¸¿Þ¨?¸öç?Â,ñ$ÅÝ@¬ž#lÓ@[µ³U­¿Å\ÿµW¿èOÉkï<¿é³^™‹¿î‹1¬Jv¿ïò<'Î{#¿È³çcQAGNfsrqTXS 1933+655?ïÿp"q?!³tR^P?±ïqÌsi?!³tR^P`?ïùë9ø?b	½›Jë~?HSÃñ¬?b	½›Jë}?ïŒNCé(V?"UŒ½ACT?Œìoµéð?"UŒ½ACY?ïÿ§†ÃÃî?S´Ý\
2?Ot°?S´Ý\
E4FGL J1934.5+6139?ånãMà?¦@2Í=B€®À;hIóiÈÀ<¾ÀÕGő@S>€ï(Â@è"»ìª¹?Ñ*—ëè?Ívñä^cã?ü4#óûÿ@æüõ‰"¿ïý–Þÿ)k?ïÿËô_¹¿Ú#½l²†¿è}}`ݐ¿Ú)À£s¸	¿ïÿG=¬2ùAGNfsrqGB6 J1934+6138?ïñ£P)}?c%NIWˆ¸?\¹_Ë­s?c%NIWˆº?ïø@Öñ¨?eÆkg&‹í?Nÿ¬¤9]×?eÆkg&‹î?îç¯Ã&?–Ã:8‡º?¡…ÏýžF?–Ã:8‡º?ï²Ðe3wb?qÕ7ÁT#c?ƒKæ³"'Ð?qÕ7ÁT#c4FGL J1936.9-4720?ècT˜nÀ;ޜ)¦À9¦óp.À<
—þ@ ¯K¿F&€?ûé{DD?±¿jŽ",ó?¡¥ÓÂ=v?ò¦ç•¥ï@œO3™àf?ï{ˆA'¿¾Öh¬çª¿áJÕù¿Ô~Àdß}©¿ÝÊhÙÞ-G¿ÑÛR6-¹wAGNbll3FGL J1936.9-4719PMN J1936-4719?ïþ'+á·t?ѹ:®b?&íAäˆÐÛ?ѹ:®b1?ïþ4‹6Úä?F£GkÌ|?,·L'Qºõ?F£GkÌj?ïõÓröÝB?Y3ò…ò£¢?TYE{€?Y3ò…ò£]?ïüg¡1Ѐ?.ÅÙÄ­ÄT?<Âöq{þð?.ÅÙÄ­Ä)4FGL J1937.0+8354¿ïñR\iud@9ÄdE#öÀ:úôàM/À<Ì+
|À@ð?S	?ÿ"Ñ‹xn§?Ċî[ôt?Á·ƒåRT·?õA›«Â'@œ¶×Âõ?ï§W\Þ'h¿àÓC>C1®¿Ò8¢]ã`¿ÞpGüó¿ägûnj,¿çã¡àø0AGNbcu3FGL J1935.5+83556C B194425+834912?ïó-ç^¾?UñϒJü?Y¤à1B†?UñϒJü?ïú×YÇw]?ZRù"ìÛ?D¢˜â"ŒÝ?ZRù"ìÈ?ïÝ	õòC?vB·õá"?q{9ß2?vB·õá"?ïYDfÊm_?yöGïrñ?"×s&²T?yöGïrñ4FGL J1937.2-3958?á6M}§ƒ?À9]&ú?̟À99­feÀ;ÿ<ñøÖ@@8xž!h°@è÷QÕ?±‹è.ú?²n¶l
Da?úÔní¥,@ͲûÀU¿Æ‹&ú•²Ú¿ä_ÿD]Å¿èØ^›–ÉÜ¿æö)	€¿îH' XÐ|¿ïµ*Ÿû AGNfsrq3FGL J1937.0-3956PKS 1933-400?ïýK¡ÆQ?1ãhÒMeH?5§ñÍrC?1ãhÒMe\?ïþ@AR?LI9ÓøZ»?+ûê×,…?LI9ÓøZË?ïÍe"›é"?uïË}T=C?yM62>?uïË}T=H?ïî"ÕH4?R,Y-Oô?a{÷*·Êß?R,Y-P
4FGL J1937.2-4217?¸–p°âޙÀ9óôým~‰À:ŒÆˆåí/À<pŠ:N@Mš{õá?ÿ ö4¥#;?Æ'7RQ±?ֱñðþ@
U°†E(ÿ?ø6+|s?ïsþÕ]•¿àñ
™¶õË¿ØŸ"ðoê¿æ¿ÞNÕP¿ëV&x¡Q¿ðAGNbcu3FGL J1936.6-4215PKS 1934-423?ÜÚúw2?ÈÈ6h¥?áøò''Äh?ÈÈ6h¥?๺‰ª?Ôß_"Î)K?ތ‹üíØ­?Ôß_"Î)K?×C~o¹ª?¼±t-:~?ä^@ýÈ#+?¼±t-:~?Õ)1s¬—?³TDiÏô?åukgF)´?³TDiÏô4FGL J1939.5-1525?âv#£idÀ1säXÍÀ:l`´u½òÀ<ŠJq=Z@¹UÐ-@ò…fîW?ȳ¤‡´??ÈÛؘÝÜê?þ06(°ù2@/~UñN6?ïá8ÿûÎB¿Ã
3µŒ¿ã% ¶Xí¿ê(ƒ¬ÈJ‡¿Þ.û–
óß¿ïÿÿ" 5•AGNfsrqPKS 1936-15?ïðÁÏ	7x?a01H®ˆ?^|aí's?a01H®‹?ïýÂDð?XyrµÏ·¾?3'í߀z?XyrµÏ·»?îdX ‡h?´¨§¾?©ºuÿ‰|?´¨§¿?ï÷×$ȝ??ê‹ËJ$d?PQ¶nÅý
??ê‹ËJ$'4FGL J1939.8-4928¿ïu‹$ësßÀ;äÿëJwÀ:…¯	ëÀ<ƒ€Íù¦@þ£NÏ@~â¡Jh?À(ÁÕ¢ß>?¤3Ê7-?怮¡=§Ö@¬¶`?ïØ5jÀ¿å+îÑ"2¿ç$aß(ì¿ÐÕbÈw(¿äÆ>QÊM¿â™ДØjAGNbcu3FGL J1939.6-4925SUMSS J193946-492539?ïþË:ô¬3?>7¾–Ñ#?#LPµ<çY?>7¾–Ñ?ïþ}Ž´"ç?Eœ¨6
œž?('·±'#?Eœ¨6
œ‡?ïü!"uË?7¦qüŸ?>ódQª¶?7¦qüf?ïõ2°ö'?B)¹?U›ôžúu?B)¹4FGL J1941.3-6210?­›H3ïªGÀ=‹*{ԌµÀ8	j#ŠHÄÀ;½G²Jk@ÚN#yÌ@͝€Ú†?—ËÄLJ±?±­­ê‰@»Šãq*@hŸô|"%¿Ä|1>fm¿â΍âVKç¿æK<>t°¿å{f¾%7¿è-••¿ì®Ö­ _AGNbll3FGL J1941.2-6210PKS 1936-623?ïýBì)«?'¥Š¹¢ò?3螲£³?'¥Š¹¢Õ?ïúz‹å•Y?ZN³c«£÷?FÐiªŸ›?ZN³c«£ü?ï؀UD%õ?vî"Ã=?s¿Õ]íð?vî"ÃB?ïÿºS9=þ>öj)?lÃß?k1°€M«>öj)?lÅ*4FGL J1941.7+7218¿êwìw•u!@6©£Ò؀À:J¤ˆàä²À<¢—o@Í Øè@|lb(ê?È°`¢|?É2ØÅS†»?þ0¨ú_­@Ÿè)Ê~¿?î¼#Òm¾¿çk6#¨|¿èÏa!Xi¿ìn	"&¸Ñ¿ÔÅ
á…k¿ïÿ]þ¸Ø#AGNbcu3FGL J1941.8+7218GB6 J1941+7221?ïñ¶ë‡æ?eÇf\2_~?\')Èð6z?eÇf\2_~?ïü펚X‡?Nå}â_ia?8"‹-;Ìz?Nå}â_i]?îK!̶eñ?¢ÉŠ (õ?«Mã4™¡?¢ÉŠ (ô?ïü"$ȍ-?0X¾Aͱ?;fÙ»–"O?0X¾AͱÌ4FGL J1942.1+4011?Îhüd.'©@ ¯'Àa"À:¥]òú^À<^úaZŽ@µÈNbä@õ‹$‹Ðƒ?Á7ÉðÏ`?¼2^½¶Á?úƦå²@IÊS˯?îOd1¿Ôʍ'_d¿ã?Èl뻥¿Þ°¾ä¬½c¿îÈi[
lÐ?ØÕÔ]dßÿAGNbcu87GB 194033.4+400351?ïé4PãQð?b‡,Á"–?f˯®_?b‡,Á"?ïùzá*1ò?eÊ;öÉ£?J{W8>€?eÊ;öɦ?îÿ¢8c~W?—:¾F";? ÜyÈ¡?—:¾F":?ïæÖ£‹g?X¶†ØçI?i)\tè™?X¶†Øç?4FGL J1942.5-5827?ì-"4ÛÀ=rˆXÿu—À:ÆGœvìÀ<'§4ŒÏ‡@ü HtãØ@D¯ñ¥Ê?ÈA¡µòÁ?¨ÆÍYd >?áz`ƒÎV:@¨L!Á›Á¿áë¶!d©£¿è¹> #Ìc¿àŧ߭z!¿×šFÓ#(#¿è?`Ónu¿ïÿÉ¿&FAGNbcuSUMSS J194224-582824?ïùŽÆñ^Þ?K÷÷;Á	ì?IÄä:"'É?K÷÷;Á	ë?ïýåeé1ö?GŠûF?0ÔжpTÿ?GŠû0?ïʔ®AVH?€½éf+D?zµ¨ßT܏?€½éf+C?ïï݂YÜÕ?Mˆ&Á_Ø?`"}¦#+?Mˆ&Á_è4FGL J1942.7+1033¿ÛÀMõçéÀsºc=¼úÀ8'%³ïáÀ;\Ì.A\@ K媔=º?ýWo£&
V?¡D{@N_ñ?ž@}@¢?ý™œô˜@֛Ž¼Eì?à@%‰ýDd¿ÓošÂŽ…i¿ß¢Š# ï¿Øae?õ¹U¿Þߟ!î½8¿×Õó¼ûžqAGNbll3FGL J1942.7+103387GB 194024.3+102612?ïý×?4Taq©?7‹'Cïw?4Taq©Q?ïüV•®×µ?ScR¥£l?=KR‰BQù?ScR¥£f?ïʓ»§?'×{K°?z¶w"x+ž?'×{K³?ïébrù?Xáٜ§Et?fðᝍç?Xáٜ§Ei4FGL J1942.8-3512¿Â"/œúPÀ9!zg¥*ÇÀ:˜£ÇðÄúÀ<7β€m@ôÃ@Z±'Ýãv?Æ-Èe4L?£"k­"8?ÞÜþ3!@@
2žb×?çQj‹¿ß]Ò®Že¿æjußÖó¿Þe¥
æãϿ֘…·d†¿ìƒ<àÛødAGNbll3FGL J1943.2-35101RXS J194306.8-351001?ïúºÖ"[á?=öN45?E§v|'?=öN45'?ïþ"í_!‹?Kp^ìågó?-Ñ*
çWÍ?Kp^ìågä?ï𭵄FH?j5"Ippû?^¤"÷sl¿?j5"Ippù?ï÷ʊ‹?>\®ã–«Ì?Qüjêéà,?>\®ã–«Ÿ4FGL J1944.0+2117?֎{ÖöRοõ
WqÖÝÀ9Ÿ©,£ÍÀ;¦I†[Ï@#Lo'*;h?ô…UÅ.rÚ?Á`Ü8Ё?Î雥"c@Û£)eT@~¿[5z¿ëgÑÀ§zƒ¿ïé†@÷A?ì~ò¹Æ_Ë?ïýßÿ¯x(¿ÆØB¡»&¿ÎÅͪAGNbcuMG2 J194359+2118?qý{?¥®
(dҋ?§gï0(O?¥®
(dҊ?îÎ>Ûe?¾±§€[½?£ÌOé«?¾±§€[½?ëöÈ'Ô?©âQTûò?À$Üõö°?©âQTûò?ï»y*²+?xdÑðÊì?!µS{5G?xdÑðÊí4FGL J1944.2+3921¿Òâg–¿X,@V#ˆÀ:5ƒO«8þÀ<+øàQ@>c†ã£?þG.¬?ÀyF¨Zý}?͐ÉE.@ßkã}é:@%ˆà%?ï¨ÙÞ-Ga¿Ô¿·%Á¢¿Û7'"Yœ)¿Ù ºKâ¿ç0²ð'´{¿è֔aKtsAGNbcu3FGL J1944.1+391987GB 194223.9+391242?êbŒ<ewÂ?¾0EöéUn?ÆuÏj ô?¾0EöéUo?ì·%*—x?ÄES*øIJ?ºFÖ«D;'?ÄES*øIK?éí~ÙöÒ?³¶,£§;ì?Ë°J˜$¸?³¶,£§;í?ê.B}YÓ²? g41x'~?ÇFö
˜±6? g41x'}4FGL J1944.4-4523¿Äî'UWü;À;ãü–þµÀ:òŸÅ,ÅÀ<aV"@!±ð°.\?øœ5Ċß?ÃoKè5Þß?À¤AhU(ü@³;–¯Ž@K-Kè‹Å?ê9!°:?ïÎ~T–Z¿ß€ aIq
¿È"CÄOû–¿Éö$_ó/¿ÓóBWhrAGNbcu3FGL J1944.1-4523SUMSS J194422-452333?ïõßNÛ?SŸq©[ÐÎ?TAcÙøLà?SŸq©[ÐÊ?ïû™¶éý»?c<lò'fÛ?A™$X	Ì?c<lò'fØ?ïßpŽŒy?r®¨#Ç?pG÷¸¹Ã_?r®¨#Ç
?ïÈP"Lî?kôtHxVz?{öWîو‹?kôtHxVx4FGL J1944.9-2143?îÀéxS•™À5ȊGìÿÀ9:._ŽÛÐÀ;݉à¾ò@ di¾µ‡â?üYÝÁç–?®JícÙª?«>Ÿ'ª?ÿÛÇ4Ý@y؜ŽÁy?ïíj Ûç¿Ñ*Ÿµg€¿Ùêã"ύǿԠº $x/¿á`‰þ#r¿Òr¬ÅÆHNAGNbcu1RXS J194455.3-214318?ïÿbÆ@ÓZ?)Z
¨©?§7å"Ýæ?)Z
¨©Ú?ïýG•Wq?Pßb—ÌmÒ?5Ç{UDq5?Pßb—ÌmÏ?ïìZ2½+?h)ywUÃç?c¥ÍBÔø
?h)ywUÃß?ïüÂÅpŒR?-Mːöز?9éÔ{pU?-MːöØÑ4FGL J1945.1-4007?ÒpöŸÈ'©À:Þ*<êlÀ; κÖ¨À<¾€íÑ)S@éé%Lk?ÿ^½çX?ÑÑT›ã Ï?àùJn¹?@ê¢þ)q@
u?Öڗ¼¿ïÿÐ?sŠ?ïýáAÎ×i¿À¸™¹úã¿â–Æ ¸Ç²¿ïÿo·HJ?ïçh5'‰AGNbcuAT20G J194519-400557?ïð=­)0?cÐþÍah?_߄¥­ ˜?cÐþÍai?ïò?
?p#?~"·´@É"?[å¸?~"·´@É!?éFñ"u?´OšU³å?˶ä9®+±?´OšU³å?ï½µ|^Ã3?sŒ\2?€' èO3?sŒ\24FGL J1945.5-0153?ï*[¾ë–yÀ)È
°ö­À;!C|V'´À<9.¿0@>ßôñ"@ݼfM;ó?Õÿ\÷§Â?âQýŽ5¸I@mczù›b@ÔQpµõ›¿íسà¢ý?ïÿÔqܼ¿¿‰c˒¿êDm'ºZ¿ïýibDBпàÇA<á1ßAGNbcuPMN J1945-0153?èVèA!g?Ȇ¿'?Τ^ûzc®?Ȇ¿?䮞²$÷(?ÑNîcá
`?֢›¶¯?ÑNîcá
`?⮟å¸Ð?¼ã‡ðEJå?Ûþ¢À4Ža?¼ã‡ðEJæ?àHQþ¹…›?¸¤œm­í1?ßo\ŒôÉ?¸¤œm­í14FGL J1946.0-3112¿ìõbŐ
âÀ8'ÿ.Hè§À9wQŸ/ÐÀ<	ûï»@r*$Þä@•a[dª¥?²&rÛiȜ?ƒNcnÝÙ?ѧé=›Áè@#â~å¹-?À~Õ]•¿éýaw¿ámÔº.¿Ùˆdà
—¿é:aûš°¿à;š{pdAGNbll3FGL J1945.9-3115PKS 1942-313?ïσ]õÈ?{ÝÐ[­¸?x>Q@=?{ÝÐ[­º?ïûô?N=?m–YH2?@/ÇïD?m–YH2?ï´"ªc†?… ÎLäÍL?'÷U\§‰?… ÎLäÍM?ïå¼ßû?[Iå
©iö?jC røU?[Iå
©iô4FGL J1946.0+0937¿èh£Ì™ôÀõ@‰]À:Ucé´d À<DF€íÑ@ D§•ßc@ÚõýG¾Û?Áò¦%C0?ˆäŒ1&=¬?ȪJè\@O7 «1¿îAÎj[¾?êÞæu¿ãŸD(y¿Ù]$~£²¿ã·/+H¿â(TÐAGNbcu87GB 194328.9+092856?ïÝø¸9ÌÞ?kfÆՓÏá?q£ã'l?kfÆՓÏÛ?ïú`3".Z?` šûMlÆ?F1¯F•r?` šûMlÓ?ï´èΗ³8?"[7É×\?'ÅÌZ2?"[7É×Y?e×ß?|zG€'?ÞæŠ=?|zG€"4FGL J1948.3+1207?ïùõdú% À.Ü ý¦‰À:ˆ­Ú™>*À;ô"ªlO´@±)bNÿ—@=sãýjú?҉Uê`o?æ
²
©§@/'…€!@BZœ¿ê?é£%¿,P@¿ã÷æV
ΐ¿àüÈþau¿êèNòÄ®¿í¦i³Ê¿ïÿâ–é¼AGNbcuNVSS J194814+120645?Ùøˆª—v1?ÎˍrDð?㻪´Dè?ÎˍrDð?á©2†°Î4?Ò/´'µ2?Ü­šòžc™?Ò/´'µ2?Ù¦
Þ³í?ÀS€QÌ}?ã|¬ú¦
?ÀS€QÌ}?Þ£|të?¶ÓXI»Zæ?à®vÁøŊ?¶ÓXI»Zæ4FGL J1949.0+1314?Ý$SüÑÀt/è%çÀ9nç¼<[ÑÀ;˜Çÿ²|@`M"ÃÌ@ïÃqÚ7ï?ºþy×ÝL?¾eà¦@æ<$s|Ï@›®] ïú?ìö쀜GŸ¿ãÿ!é^ÓË¿ãtßp=½¿çIH¾H¦¿äé0&Ž¿è¥
±3êAGNbcu3FGL J1949.0+131287GB 194635.4+130713?ïbŠBÿ4$?•>+ [«?"®· {L?•>+ [¬?ïÌWÙÃ?®…\ÂòÍ?Ÿ&uÝG—?®…\ÂòÍ?îÉ_³"?œÂP"LR ?£jTÎÃ?œÂP"LR?ì‹kÇKÊ2?œ]Î÷0×?»¤¡Å¡®i?œ]Î÷0Ö4FGL J1949.4+1247?ç%³Hw%ùÀ©Oð\À:‹n}ŒÙÀ;¹rl.'@ŸœBk_u@gFBÐ_?Ð1Ñß0Q¬?ÂÊ7F=Q?ô‹Ëz½5€@®¡É=÷¿ïü2¶5±"?ïûçÂq¿ä¡>iÈ¿âÄî|Iýz¿å±[Ývh<¿ïþñ­VåÀAGNbcuTXS 1947+126?ïøg։?Q‹p¿p?N`¥Û£ÔÐ?Q‹p¿j?ïþ]0Cš?P>[-ð¹?*,ûÎ&|‹?P>[-ðÀ?î|׋tv?ŸU<ýýo?¨2‡Nȸˆ?ŸU<ýýt?ïê̈́›R?YTõü'ß»?e2{d­ï"?YTõü'ßÃ4FGL J1949.5+7311?ÁùU`a@5ÕU>öµÔÀ:WçG¢VÀ<݂ýuâ@Ÿî)†Œ@͒tâ*,?®Ãaéÿã?¿Ú®ó׏?üØþÒ—@Nޞ†hd¿ß¿1×JÕ¿æêG1ù¿ç`N‰Ðκ¿çXjû ¿ïÿÏ=ÀTï¿â"h\૧AGNbcuCRATES J195016+731028?ïæÔÓàÕ?qDvô^Ì´?iî+,+v?qDvô^̵?9Y<p?¡¯["?€Ù©°ùãà?¡¯["?ï¬õæ3Ë?ƒøþN"Dt?"†s
?©?ƒøþN"Dw?ï4'Gh6?ƒ¦
ì²W?™m·ù?õ?ƒ¦
ì²WŽ4FGL J1949.5+0906¿èæ>
>SÀ!? §?uÀ9·
Ø/×^À;ýžvx,@ X醖Ý}@€©Þ‹;?¶"ÁI–¢¿wä
¨‹R?Â
]v'Ï}@
$ô)Ýôè¿Ô"mè2Ú¿æô¸Œ£è¿çÏ
Ÿ$óÕ¿ÍHuûìÊ¿Ýqœ¥g®¿ã=ȝ"#^AGNbll2FGL J1949.9+09071RXS J194934.1+090655?ïþMþ";Í?!Ä~QŒ‰ä?+ ÌC#ø?!Ä~QŒ‰Ø?ïþÍ.ÿ²?DY$u.÷Š?#-ß²?DY$u.÷|?ïõ~æ'?bÐ4'®Y?UÙÖ2ÛÔ?bÐ4'®_?ïüêݛš?*ò‹–Îl?8©#/ó9?*ò‹–Îl4FGL J1950.6+3456?×ô©8V
@&!`¢ØÀ:±îX7ÏzÀ<.ʔ
hž@!P¯ýˆ¬?üâDhå?Ó«'Ëöãø?ÁP±ˆÎ›.?÷X¨ø².?ÿG˜ÛX«¾¿ïþ9áùâ?ëa±Ë¿†"?ïü¾A™¨]¿ç(Îàù)¢?˜!ìf#¿éßÓÚÞˆAGNbcu2MASS J19502776+3456224?ïðfšŸôM?c9ßßE3'?_2ÊÀg"?c9ßßE3?ï­ZœÞ…Ï?¨®ÕN?"©XÈ^Œ^?¨®ÕN?ï9öŠÉå?'ø
CŽ%?˜Á.¦Ã]P?'ø
CŽ"?ïW–~rà‹?‹‡ªÖÂ?•
01£î^?‹‡ªÖÅ4FGL J1950.8+1211?íFïŠáÁÀ!úvSCtÀ:دYÀ;ȟ·ÀÌ@,Ža'&@û
z<A?Æjt!?݂Bdÿ^@ítýØÞS@°7êê¿é°ò¡G¸Ñ?í˜{V¸sy¿ä–ù¬(è¿ç(ÒÁ&¦¿ïÿMéDÓ¿ãÒ ß²CAGNbcu3FGL J1950.2+1215NVSS J195059+121316?'Ä?r?•i§úÄÄ6?ïw7Iß?•i§úÄÄ6?·¾R<áïY?Ä»'¶%?í5¸cÂ?Ä»'¶%?¨2×
yR?˜"áP¤Ø?î|Þr(l?˜"áP¤Ù?³HdKS?lÇâ……?í–ÿsv?lÇâ……4FGL J1951.8-0511¿éÌøPá7«À/–¤D‡À:Mqåöi~À<¢Ô«¾_@܁Ðz+@)2^!‡?Ç*ÖØ¿IW?ʘD/ùŠ@¼]\Òi@8lýv?ïö¶^Ì>¿®^‹{ž±Ü¿ä«¤=âc¸¿ã_Cý…Ò<¿ì]2K­¿ÏÛ¨ï³AGNfsrqPMN J1951-0509?ï(Šé£=
?š*º7É?šî¢Ë˜^ß?š*º7É?ïü"Ù&+?Uô"w?>ë6ΩC?Uô"f?ì 
+¼Ô¾?¥ªÂêœTÑ?ºÿ–¢Z
?¥ªÂêœTÑ?ïå¿ÛjÇ?W¦F3,§?j@ï$•8n?W¦F3,¯4FGL J1953.0+7651¿æ0ª}èE @6øäd™ÍÀ;TÍ
à-ÓÀ<±
?x@k w™¿"@pðÀÇÛÌ?ÐÙÖÀÁ{¶?̓{~% ?ø‰Z¼äø=@ã…"¿¶?Äßbцp?æ
ÇNފ¿ãxÔ'4!¿ÛŸ¯È°š¿ìô_î} ½¿­s£æ¤AGNbcu3FGL J1953.4+7653WN B1955.4+7642?í³®?{4?«‡ŸDô'î?²bŽ'ni?«‡ŸDô'î?ïËäöN˜?—1ù®Zz?z
"س¸^?—1ù®Zy?í©¢S‡þU?¡G!.éL­?²²ícÀ
W?¡G!.éL­?î¡VÕ؜?FΦ=(?¥ê'¢v?Á?FΦ=(4FGL J1953.0-7025¿Çw"µIÀ>–Œi/nƒÀ:PYddIÀ<eî \+z@îl"¸Œ@vg=%û<?³ÆÊ¿¬RÚ¿©§Çà	k?õÓ	AÈ!l@õdW"¿ãc¸6<Òï¿Õ'šCÅ
¿æŸ¤¯rÊ¿Þ½Ÿ
ò¢¿ãžlґ1ì¿Ø<åcœˆAGNbcuPKS 1947-705?ïìI4øSG?WZ$Óu†?c¶Ë¬¹??WZ$ÓuŒ?ïñóE8?sèÈOx*È?\Ãuòÿ?sèÈOx*È?ïÛFdY?x9[›É™?rq\øMӍ?x9[›É—?ï•¡†é?tS;ä Å?Š¾—¹ÞEÂ?tS;ä Æ4FGL J1954.6-1122¿Æó7ka¸|À3 é_ªŠƒÀ8çDŽ¥JÀ;Õ¤xð¬¦@›jT1°@YgåÂg?ª—Àâ™ú?®¬Bn~R@±!«KrÅ@¨sÿ¬*¿Ã£]<Ç¿ä%"?]ä¿çšÁaߙ¿ã(ÛPN¿çd×Oݍå¿éÅW ºJAGNbll3FGL J1954.8-1122TXS 1951-115?ïý93±ÈÕ?/ËÀ+€Î?66bq¹_Y?/ËÀ+€Ù?ïü6f¯?ZÈâ æ?>Ooüʈ2?ZÈâ á?ïËB!90?yˆÏÍùÀ?zxÞïcgº?yˆÏÍùÂ?ïþ¹÷Çåý?"K‰5?$`ƒ D&?"K‰]4FGL J1954.9-5640¿À—ÁÃ|!À>ütÙÆ°SÀ: ó9H *À<`Ñ>K•*@ mIT1Ûo?ÿ*.!{zË?²yOa½	`¿¢kÁo Ÿ2?ñh'iIo¶@RÉÑoÊ?ïقˆŸ¿ÕŠûœ$¿åÕ¶`#× ¿Ú_á§Oe¿×LÕ[;ºì¿Ñ¿LF)¯ýAGNbll3FGL J1954.9-56401RXS J195503.1-564031?ïôs¨u"a?VÖx?<]?W¯Ù?ç?VÖx?<V?ïü$éëè?Sö3ᗞ
?>Ø·˜ ¿Ø?Sö3ᗞ?ïÝÖÓùu?uw‰xô·É?q–vƒFa?uw‰xô·Ï?ï½u´	À?i5õ=—?€¢'ý¸Û?i5õ=4FGL J1955.1-1604?ïþYiÔ À5%ð=]…À9¨èÄ3¡À<MjìÝä@ 2ót'Ý@8S 8"¬?²¼ùÅÿ(??_£Ê­à—?²~9|§›@éú8•Èª?ïoAT©P¿çPB7²ô´¿âI>¢Òþ?¿àÂkµZÀ@¿ßì.Ý
6Ê¿Éæf%ù¹ÀAGNbll3FGL J1955.0-16051RXS J195500.6-160328?ïþ.éÁ?(`§pZŜ?-oÃô®?(`§pZÅ?ïþ®IÚ&?F·L:ßQ?%n¢]šŒ?F·L:ß\?ïônPҒ¼?bÏ.|³È?W#^Zچh?bÏ.|³º?ï÷Cüæù?@q/Y.Ñú?Qx3àò?@q/Y.Ñú4FGL J1955.2+1358¿éÙº©Ë\ÜÀAÞÑ·À9å½^šÀÀ;¶UNæíà@ÂІ×}@6ï›-îP?¸_ðU"?ÇhóÉæ¾f@
'¾}~°à@¸Wï«&?­3!8E'¿äŒKÓ=)V¿ä$"Ÿ^Õx¿æö`y½[@¿éœ#î¡¿áüŒéAGNfsrq3FGL J1955.1+135787GB 195252.4+135009?ﶝZëý?€'Ã-i?'X©X…Ú?€'Ã-j?ïû;B\Ã?`ë#Dy->?C÷²ŒóÇ?`ë#Dy-;?í4'‹më?¤ŽVæÖa"?·ž[뤐¡?¤ŽVæÖa#?ïûÙì¶?0O/7ˆ(?@˜M'"¬¬?0O/7ˆ(4FGL J1955.4+5132¿ì˜mŸá@'šoÅåÀ9†¸UFƒrÀ;ó€`°@m"M¥$g@çç†w~?¹Hw"^?¿†Ñ™»(@²¬ûv-"@õäÇ|¿ã¸×í'?2¿âüÕ©¿å›À¿èý,)Bï¿é'ìKî¿ïÿÿ&¦³AGNfsrqOV 591?ïû:Žðç¼?@òÜç)ô?CÄ<aï?@òÜç)ø?ï÷Êgšö
?sÎ)ÖF?Pk0Êä×?sÎ)ÖF	?ïˆÉp°Ã?†ÇœÊ5®d?Í£úÏb?†ÇœÊ5®k?ïöŒX?DŠPp°?SÂçNåÑ?DŠPp¢4FGL J1955.7+0214?¢tÌݘ…À*l´¿ÍhÀ:D÷m5ŽÀ<$@µÒµD@!F0¿:'ù?üïçžà*x?À«˜Ÿž–Y?·A©ÿ©&?ü\6@'¥LUC(¿Ù=ªðÙòO?ïû¨LºÃ¶¿Ð"yA4}¶¿âñÃA2Ð7¿ØßÁœ"[¿ØqMJ5®AGNbll3FGL J1955.9+0212NVSS J195547+021514?ïãu}ŸÓ?mª€UDåR?làŠ'`,ä?mª€UDåX?ïȉ†¬`Ð?"š¶Z%Gö?{»<©Ï—¬?"š¶Z%Gö?Q1DJ?‰à÷'Ò+ÿ?Õ«³®íu?‰à÷'Ò,?í¶ Ä÷‰L?œ¦ª×w»:?²JùØCµŸ?œ¦ª×w»:4FGL J1956.1+0234?Ø"Í;T]ZÀ*EóFí$À:Æ3\MÞ°À<8x{;à@ O¥ï?ÿÂÑ¡GãÄ?Ñd£Ã"ô?ÖW»þžV@FÚhµÌ@ó¹Qoß6¿ë7¯ß/j?ïõŠ@`B`?ߺl¢ë|æ¿Ø8ÝâHßî¿è¯¯…")¿áçÀÃÿõAGNbcu3FGL J1955.9+02122MASS J19562808+0234250?ïŠGŠ©Ii?"nÏ´Àµ?nU­¥¯?"nÏ´Àµ?ï°ÆEL?¡sgžÞIT?ƒÎn¾~,õ?¡sgžÞIT?íþãŠõ?¢[ù%?ê¤?°ç+¯PO?¢[ù%?ê¥?íßñžôà?š°¯"C
,?±sY?š°¯"C
,4FGL J1957.1-3231¿ß	aÏ>øÀ;7¼ä!}(À9üŒí¹¬À<? §?u@r⪯–†@–äÛ·K[?ºò¿¥œÝ?€{ ñbê?À—Á'R)n@	œp›ôgÆ¿ê b‹l¿Éy&‡~9¿ê$º"¦¿æÀ!ß&¡¿Ýsb"^úŒ¿ïçH®ÅzÉAGNfsrq3FGL J1957.0-3234PKS 1953-325?ïù~âex?OWà{]\?Jvjßx?OWà{]U?ïþîA7—?:R¯…/)ô?!;솒?:R¯…/*?ïdêò~.[?Š'ÓÊêÕ?"b¡°:4¤?Š'ÓÊêÔ?ïýGzkª?+©1]³!Q?7ÍÄ,¢¯?+©1]³!l4FGL J1958.0-3845¿všª‹<ªÀ<öÄç%>À8P®{¨îÀ;«Ãæg@·RO@kÉÂbæ?£jåØÛ,?ÆÈ"D"š@"Ñ»IÊG@e:ÂHº¿Ït"çÙ´¿Ü¶}Àu%œ¿ä‹ÿG¶¿æ´Ka'bE¿ìO°â‹zó¿ê$Ɔ"ÄAGNfsrq3FGL J1958.0-3847PKS 1954-388?îfÞ•·Å?©›)œ}?©'¤ƒ¨?©›)œ}?î©&ï÷V¶?½Þ?µ4r×?¥m'Š"¯?½Þ?µ4r×?ê÷oà½?¯MŠH!z	?Ä!ûž@}?¯MŠH!z	?뮌pï?®Yþ
ó-¬?ÁEÎ?‹ÜE?®Yþ
ó-¬4FGL J1958.1+2438?ëŒEâÀ"À8*»À9Â¥Ξ^À;î*ëf@!,çƒ1xH@[GA1M?»1±×(¿x}xü–'?¿Ñm_BÊo?û¢ÝŠµ%;¿ï'Yԇ¬1?ïÿ…¡•ž¿ÊÑÖâOj÷¿äWF¾*rš¿åŠ ½zIr¿ù[1e8ûAGNbcu3FGL J1958.1+2436NVSS J195800+243802?ïÑ\¬Þ4?u¨úŒ¤?wxQ©æ¬?u¨úŒ¤?îúQyÀ??½—RÊP²? ^ºècü
?½—RÊP²?îÓ6c\†P?—>ŒœÌú?¢Ì™Ê7›?—>ŒœÌù?í<Šü~'¨?©ö$ˆOf?¶¨rÃ?©ö$ˆOg4FGL J1958.1-0711¿ëÍeà¢ÄÀ2Œ?>À:¼áÑ@ÏÔÀ<SbI¡3Â@ +Ôíˇ@_…Q
8Î?Ç{×ómK?¨.ÀÃæ/†?㍷ä{õ@۟@!®&¿ã—ëy`>.¿è3¬jVµï¿ã†Å~ð¡¿Ó:Êi²K¿ãkùM^X¿à½ÛÍñûAGNbcu3FGL J1957.9-0712NVSS J195801-071348?ïÿ^"‡à?q_c¦A×?-}oÖË?q_c¦@å?ïþ¶÷CÙ?D9f?$Ÿ‹Âcµ?D9a?ïü#o…ç?=Ö êÐOà?>礃ÐÓ?=Ö êÐOâ?ïý6DÑg?'@¬ÄK?6MßátČ?'@¬ÄK<4FGL J1958.3-3010¿¢%õ»SÐÀ:È-œñ<ïÀ95íKÈUoÀ;Ùý2Æ&@ àZX?ý&ú@£^?¯ ö° Ï?˜ð|C6Oa?ì¿ÓÀí@
íœûù¶?ïïíJ.¿äÞv]Tní¿àR0N|e¿ÒžnÀ}¿ßœdпÕb¿¤(AGNbll3FGL J1958.2-30111RXS J195815.6-301119?ïþ¦Øô?·65%4?%'wà¾ó?·65%T?ïþ32'Ä?L'yàçž?,ÌÞ6Óß?L'yàç¤?ï_?nHÑË-É?aüSaô¡™?nHÑË-É?ïú‰›8òã?5Ôô5o_D?Eٓ4w¬?5Ôô5o_54FGL J1959.0+3844?â@Ȃ¢*­@%/<-­¸À9Ëx²Õ«À;'š0˜N@@q€»QO@1^aµ&¾?·¾Þ!³Ú?ÓUÃW@Ü
²p*@>3U—â	¿ÛW4ó&Ô¿äL#ú±¦¿çT¥ÿX:¿äô1•¤A"¿ïàñ4ˆs¿ïÿù³>†AGNbcu3FGL J1958.6+3844LQAC 299+038?íôQ:êeØ?°³ä˜2 P?°]v(¬ÑD?°³ä˜2 P?î V¦¦?Àƒª â1?­ú•žþŎ?Àƒª â1?ç2†¢¬Ï×?³Šæ×BjŒ?њòº¦`Q?³Šæ×Bj‹?îU WÕU?"ß‹:?®­ú'ª°?"ß‹:4FGL J1959.1-4247?àZÿ¸0À>ÚQÎÀ9]X «À<ä«ã£@÷8 ؽœ@(V£zÃë?µPNÅ_ñ?ŹH
°³@
Ár%·@ÆÈo(¿µVçÃH>³¿ÜMÍ=`Ó¿åªåò7Àa¿åÖmàXDæ¿ïS_²¿ïù7Y2¡=AGNfsrq3FGL J1959.1-4245PMN J1959-4246?ïèx}Ô?coÓíi?g‡'à+ø½?coÓíe?ïüq"oș?VŇ³ˆ¯ï?<v쁻89?VŇ³ˆ¯ï?î;g^e±—?†Âîú‹Ö?¬IŠ¤æ‹?†Âîú‹Ö?ïÿf€M^?¢;"b(û?/ÿVT?¢;"b)^4FGL J1959.7-4725?ïîÆÁ¥ÁÌÀ>Ø},{‰
À9!´:.Ï÷À;¿"(fQ@S±uƒdÏ?ù{üä?®Õ¼þ ?ÀqW†#Æ@À­Ù©@ö"Åš)¿Û¾P§ET?ñ³6#¿ÔÊ¿ÁÌh¤¿Ðï»dD£¿ß†—D¿ã|}`þÈAGNbll3FGL J1959.8-47251RXS J195945.8-472531?îžæC¿y?©ý˜‰%LÓ?¦žKÄb?©ý˜‰%LÓ?âMD³Ô
"?Ø$c{,â«?Ûev˜WêÛ?Ø$c{,â«?íJƒË/ƒ?§.¤›íeŠ?µ«ã¦ƒï?§.¤›íeŠ?æËßO;?¸¨I< ä?ÓÊhA×a‹?¸¨I< ä4FGL J2000.0+4214¿á.ÇËðoÞ@ÉéÍ³}À:-ÏZsÀ;¨ÕÑXLÈ@îd¥q>@]_V§­?Ãà™~욿 ]æ»?ÜŠ]ÜT@eLÚÏ¿ä×MÄ®ñ¿çûÃà•®¿èKÈö~vþ¿ä-RòK¿æ‹È ˜;v¿ïC¬ýúlAGNbcu3FGL J2000.1+4212MG4 J195957+4213?ïú¨hZ11?DÃßéùÿ[?E^^—;@
?DÃßéùÿa?ïý},VÍ?Q¼÷îçcW?4I—xH?Q¼÷îçcT?ï‰É&ü ?Šø™'m?¼ö@÷À?Šø™'i?ïÿiàpà?ÛŸdâ2?2Ãñãíö?ÛŸdâ<4FGL J2000.0+6508¿êŒ:?.K@1ªDØw$ûÀ6ï.¾YlƒÀ:é">¿@¸L]{±&?ü.ˆ>''ü?mJ—do?›°]ÓùE@Ô>š4@*æ';Ù?È˜=V«¿Ó¬%Ã'í¿ÚÄLÉÝ.¿Ùt-݈ݿà¯ÁÏÖ¿Ó_\òI^AGNbll3FGL J2000.0+65091ES 1959+650?ïúcþÿÑö?DmL֊Kð?Fp¸)T?DmL֊Kë?ïö¯ºß	?g–Ï	¢»?R ‹üAíh?g–Ï	¢º?ï³-"¦j®?‡|.¬Š·?ƒ4žÖeTm?‡|.¬Š¸?ïÿö—2—>Ñu³îˆLî>ÒњÐèf]>Ñu³îˆIv4FGL J2000.3-2930?çILgs¸À:þó¡LìBÀ9x>£©½ÔÀ;ýû›ût@>Kw1@‡ª4ò?²+g¯fµ?ªž,a™`?ôYè'u¹?øh5Uø/&¿ÙíÚ£úñx¿áf½+-«¿æª°þ:-"¿æ|ZYê
¿èþ»ýq°G¿Þ	5]ÚѝAGNfsrq3FGL J2000.4-2926PMN J2000-2931?ïm¶.}kö?Š"ÏâՔž?'I:0Rg?Š"ÏâՔž?íØ'™Y?¾^ã'\¹ü?±?ƒïk5:?¾^ã'\¹û?íè1&w®?¡	¸Å[Ï÷?°¾vÏdB—?¡	¸Å[Ïö?êWxí¦¥K?°Pù)Ü?Æ¢IejÕ?°Pù)Ü4FGL J2000.6-1328¿ïÿeîð:À5QÇ5ï¦À9Ãí~<QÀ;ý}K…9@ø‡Ô3@ÝS¨Á?·»júŸÃÕ?µ=ä7
?ùš£Ÿ¬Ù@ózÜÀ
¿Õ·"ÁÄO¿à®È4·—±¿è (ÿӊV¿èÓ}æOU¿Üöÿ<
È¿è<ýâC'AGNfsrqTXS 1957-135?ïûVµÌÐÂ?A"ä#(V?B¥(̼öA?A"ä#(x?ïýš³‰š?QwÐoƒÂž?7S*c³7?QwÐoƒÂ—?ï½p©¥Èè?€}»–äí?€£Õ–Åò?€}»–äå?ïÝYN ?aEߚÈ?qS|Øøð?aEߚÁ4FGL J2000.9-1748?۞QêŸg9À7çF˖lÀ8®Í"]"À;˶…ì>@Äm/ƒPW@
4†ðIª?¤®ª¢ÖY>?½[¦Õþ`?÷jÈ˶LX@P¨dÅ?ïÁcâþ¿àØÙ`ð¿åú%Ëk£½¿á4&­é²·¿èy4j¤9¿Öð-¤þ҃AGNfsrq3FGL J2001.0-1750PKS 1958-179?ïúäfßiž?A{'Zzš?Dnd'YˆË?A{'Zz¬?ïýeøŒ~è?LGdøm`?4Ð;œ½´?LGdømc?ïÕSÒoO?x Ä@U-ê?usÖÈXž?x Ä@U-ñ?ïüŽCØ¢?.âÇ(ÌC?;"á:æR?.âÇ(ÌC'4FGL J2001.2+4353¿ë—ôš8Â@t3ÿ
zÀ8É16Ù±À;7ì]‹ÌQ@‹7Ö[û?üùä"rÁ?¢¼'Ÿ<ø?¸ÄP@N¡@«â´•žb@"7Ð%¿Ýù7Ēk¨¿ÚRðÛö¿Ö2ü´›þ¿Û!ŠßlŒ›¿â¸oG¶¿áö˜ã'4pAGNbll3FGL J2001.1+4352MG4 J200112+4352?ïýño½…€?*ùK;ÃFI?0t'ÔO?*ùK;ÃFD?ïÑ/˜PÏá?ŸÎÐר`?wh3ט?ŸÎÐר`?ïÄÁá€ï?"¿R{"Ç?}Ÿw?‡Å?"¿R{"Ä?ïÿΈ™[4>ðÏ–•u>ø»³Rfv´>ðÏ–"ûê4FGL J2001.5-0818¿×i~–M6À3TFù¹"âÀ:Ш·CΌÀ<B
Ìsá@žŸä@OÒ}浬?Ä2"ý[
¿™f`ݐ?ىVá
K˜@Àû*XC8?äzfކ]¨¿å®‰J–ý¿ä{Ëóˆù8¿âÀ_C‡i¿Øyx;ûÙ«¿Ûƒ½D³«AGNbcuPMN J2001-0820?ïþG=?=Ýp'·f?.G.{ŒQ½?=Ýp'·|?ïþӌý¶?HO¶—|Ÿ'?"Ç0/ŸŒ?HO¶—|Ÿ0?ï÷|•Ÿ(?awµãt?QÕÀÁ°Ã?awµãg?ïýŠ}­ÑÂ?#…K5°¯†?3¬'qú¨?#…K5°¯­4FGL J2001.7+7040¿íûœy.hª@3õXÙµé[À:Ÿð˯–À<Mҍ.#@ùX…Ó8@ó:G#«?¸F	¤™|é?¯ãʝÑc?öGŬGH@.çÉþ;?×¼ÙûŸa¿È
‰*‹™Ò¿á7'Ô'½¿âa‡"à¿á`žü/¿çŒ:€¯gâAGNbll3FGL J2001.8+7041TXS 2001+705?ïé½¥šs?a¬ÎzÑ/â?fBéZec?a¬ÎzÑ/á?ïö*Á?hÝÿºxON?Sª}çÏ÷4?hÝÿºxOG?ïÕUÔ¨+Ô?|uÉé-e?uU«êy?|uÉé-n?ïoÙ%©]?u†eú˜FÕ?Œ¤	¶•¨ó?u†eú˜FÕ4FGL J2001.9-5737?ê-/|ÿNpÀ?÷ë[-M@À:‹¹ÝÀ<Œà«¦âW@ðDK3…?ÿÙGÏ¢j#?Á·vÙ%K?¶W´ü?öB;C¢ìÿ?ñ>¹Ôw'?ïùPMö-¿Ô]Oö¸Y¿åP
nîË$¿×[l7`¿]¿Ûû+ÚÏCõ¿ïÿÿÊPËAGNbcu1RXS J200205.7-573644?ïü‡NSæ?@=—ö–™?;ō`Ϛ-?@=—ö–?î¿«m?T
?±ÜPEÉÁ¼?¤I,
¿??±ÜPEÉÁ¼?ï±fÒ?ƒíԘn2?ƒ¦`xºß?ƒíԘn3?êîîË/ò?§zÆÑÆÄ?ÄGÐDÓ@7?§zÆÑÆÄ4FGL J2002.4-7119¿ï"—ÉWÀ?@®û*®)À:Ë«®o´À<'°P$Ü@!ªñ§L‹?ùèäZˆ?Äþ2J€ì?¼"Ôeh±?÷r¦É¢@#'+f5?ïÿÁìžú,¿îÆŽÜ&?ÞSÇÝúœ"¿È1q'"[¿Üƈåí/C¿ÏpÜÔ+çAGNbcuSUMSS J200227-711940?ïÿ‡R"÷u?x=­ÉëF?+wB"ÎÀ?x=­Éìr?ïý¯3GU?SÄóCX5?7چeÅVv?SÄóCX+?ïò÷­ø¤ƒ?e±ÿGRu?Z¤¶ûo?e±ÿGRw?ïä@¡W(?Z½4ýÚLû?k¿^¨þØ?Z½4ýÚLô4FGL J2002.6+6302¿×"ö!l@0q€²BÀ;qPþU0À<Ô®¥šXÜ@""¸;›6¨?÷¤G¨5=Ï?Ðg¼'c?ÐWˆ
€@=Óºý—p?÷ÙÙò$J¿í4DÀ¤Jx¿ïÿê o·?ð¿Ç—…BI¦'¿ÛåœFó¿ozFm!ÁAGNbll3FGL J2002.7+63031RXS J200245.4+630226?ï÷zKÙÜ?PÖCÔ¿òð?QiÊLFø?PÖCÔ¿òö?ïá<ýt?‰¢¢äÆ'?nÃìÿ‹U?‰¢¢äÆ'?ï˜é«õ‰7?‡¢:à?‰Å•²C?‡¢:ßþ?îÇ©CÔÐ?":ûo"´?£…k¿2þ?":ûo"³4FGL J2005.1+7003¿æ+_ÑV@3oÚè'®À9ðhÒQqÀ<#ñLÞÕä@ z¾©HŽ9?ú;o&ÿHJ?ºÀˌ°Ó?Å®6Jü@ÍÀ:S@ð6¿ãXò?Mé¿ÃþFïƒÜ¿ÑÂQž®+w¿Ð:² {¿ßGC…:è¿ä¢ Æ´…AGNbll3FGL J2004.8+70031RXS J200504.0+700445?ïñÑú:ê:?SËĈq³?\\Š+ˆW?SËĈq°?ïóËfÊçÍ?o©±w¹ú?Xi2j0f?o©±w¹ü?ïq·™m‡'? ¿oLøf?'ÉÒO
´? ¿oLøb?ïÜ9U—?[ƒÕÏ
?qãU{ñ´Z?[ƒÕÏ4FGL J2005.2-1822?Ô#š–‰¸À8Gà·õ¥À:YEnŸÀ<o㽪@´"¢lQ@ÜòB9`?À¡âhjx?0°[@+kÇú*(¿ÛŸ¯È°š¿çèµ`Ÿ}¿ê@bUµ"¿â
r_C¿îØð²È?çý/Á
ÑÐAGNfsrqPKS 2002-185?ï÷:›Ä»˜?S°Ê8
L¤?QŠÈvˆÐ·?S°Ê8
L¦?ïþ‰î·Al?Gò×ç~ò¦?'a‹é+Ž?Gò×ç~ò‡?ï´lÿd¥&?'ó}ŸÌi?'äÀ&Ö¶?'ó}ŸÌk?ïû†(¦v?6gÎ'{̎?Aç³]f+?6gÎ'{̒4FGL J2005.5+7752¿ëÛ¿ŽÿÓ9@6»½¯ljÀ8cSÒåë'À;ºåaïa@>®ïl4@"]ªÖ?œãàBSX?ª[<D\"@
ßE™›@¿ž$DÙ¿ÅN	¸»rÝ¿à'úáˆÁ¿ã¼Lßx÷¿á{¸<òϖ¿æÄÕA»a@¿åA".ÎI¥AGNbll3FGL J2005.2+7752S5 2007+77?ïýO–ØÀ?0˜)óhß?5ƒI9ÿ"G?0˜)óhÞü?ïøº•¹?cû5q<\Ò?M«Ç™Æ?cû5q<\Ï?ïÙ,R{¸¾?xúÐ-LJ?siÖÂ# s?xúÐ-Nj?ïþ×B$ä?ÎO(Ç<?"‹Ý±¿ž^?ÎO(ÆH4FGL J2005.8+6424¿ï8L
-B6@0Å:æ…ÛwÀ:f™5ƋjÀ<7w^@1a¼­ž@†ö¼Š_j?Á%x	¦ó?ÏWá&öå@b[T‹@Ձ†R?ïòJ¶Ýw¿ÌÞXeqÉÇ¿åêûVM¯¿ãG¦¢–˜]¿ëÔ@ßn:¿ïùö€û=#AGNfsrq87GB 200541.3+641601?í2|!Ž1?°a\tÉ?¶lŽóŽu?°a\tÉ?ïñ'$@¤1?rÈB£€Çv?]±·~·›?rÈB£€Çt?è;W>¦3-?°¹M?Ï£g3L?°¹M?ïR'L?mf,·e?•¼¯®Ö|?mf,·e4FGL J2005.9-2309?ïžØEC™XÀ:#'ˆÀ9 Á¶UaÀ;Þ{ÍÖ¸@HñS¿Å¨@19ÓÀÝ?¯XËH=[€?¹"IV
N@<êy…ýÛ@b¥ç…µ·¿ÕÅqú_r¿á.›‰]â3¿æô÷ŽAvÿçÌ.¬­¿æm¸¸ÇÝ¿ïÿülòAGNfsrq3FGL J2006.0-2311TXS 2002-233?ïÿ¼-.­>ÿ7%H6Às?ô´Tºˆm>ÿ7%H6ÁI?ïý¨?ÌÎÏ?NJÖë?2¾™‰"ï?NJÖÊ?ïÀÄVÌ h?vâÕò•ò¾?Ô™¯Ìa?vâÕò•òÄ?ïÿ¤4P>üŠ{Ý¿ý?òëú9bó>üŠ{Ý¿K4FGL J2007.2-1433¿íê›6NÇÀ79~ºñ6À:TÌ4 ˜ýÀ<'¬-ðÔ@åÅj­É@¦rÅð9¹?̍ÒfÛ)?è% }ä\`@lûï¯P?ûœNOnRC¿à
sáÏw¿Ýe~_–~¿æÁ³"¢Ú¿ï¹û8ðâ¿ËÁßeUÅ¿ïÿþBe«+AGNbcuNVSS J200711-143205?ÓWN@¡›ž?Α"îdÈF?æTX߯22?Α"îdÈF?Æ»k¢*?ÐÓ:mìeà?êQ%<:—u?ÐÓ:mìeá?Ó¹#
-è?¼ejŽ,/?æ#nzét‹?¼ejŽ,.?¥09Z©Ø?¤2¸<±¼Ø?üjUb?¤2¸<±¼Ø4FGL J2007.2+6607?Ó]H¥f0ð@1s›fù3]À9Ò"ÿ‰;À;ñgº#|Ý@¢
¢Ed¹@]e¼{a?¿2ŸÝoK?÷9½ï§@'¬'\f@lÐ"l¼l?²2³=ځ¿çòêmDŽ¿èÖÁ½Ð»¿è7çÍÚ¿ð?ïÿþR€ÖTAGNfsrq3FGL J2007.3+6605TXS 2007+659?ïòïR%?[؄u‰b÷?Z![µò݊?[؄u‰b÷?ïùÏ*0?bVt»a•?HÃWóƒ>h?bVt»a•?îò;±i³?"Ï=!Œ…? ÜFôédÏ?"Ï=!Œ…?ïìv$ºUÚ?W-%¼i&6?c‰ÛEª%?W-%¼i&14FGL J2007.3-7728¿êhSj'ÇÀ>†yF<û3À:k‹dL°³À<G¥«ö"p@.ß/ûÆ@F5~g?ÄxH:	ç?×±0@KA¿½ð'@¨žÑç¾Á?ï¿5¾§¿Ù€_ víó¿âûH
ZÍ¿èÙéëÁ"š¿ïþâßâÍ?¯aT¿Ü	½AGNbcu3FGL J2007.7-7728PKS 2000-776?îÁ%J'ü_?£¸"¯µ÷+?£í«VÐ9ö?£¸"¯µ÷+?ïò²k4ýú?†ß¬'"T1?Z›)–	Þ?†ß¬'"T1?㹧?þ|?¶ý0DH?،±Þ?¶ý0DG?ïӊ¥Ñ[\?f$¿œ"D?v:­RQÖ?f$¿œ"B4FGL J2007.9-4432¿í´Eñ_ì2À?ؖþ´¦eÀ9tÓäCÀ<€§ZL}@k›@½Òtw?³–Ç'5#ù?ÀÖ­ _@%çñ@ccK©Ì˜¿Ù/-••¿ã™*]÷'¿çèÎUcä¿ë¼[ed¿æŠX^©¿ïÿÉC«P{AGNnlsy13FGL J2007.8-4429PKS 2004-447?ïþÿDёò?ÇìÆÀÖ? ²æàÚ?ÇìÆÀ®?ïýòæܳ?R'ÃÊ­xî?7hÉ^î?R'ÃÊ­xÜ?ï´}¿Z ³?|J‹ÿÕi?'à)wÓS?|J‹ÿÕi?ïùKUîbÓ??'ì5Jb?JÒ¨Ft´v??'ì5Jb4FGL J2009.4-4849?·ú5'HÊ;À@M!…Æ~À8.C~ÚÑrÀ;g1Ԏb.@pÁñÒk?ûü݆Xt5?ŸÌØؖ&?¤"^$Bú@é%»{k±@(ýâPm?×¹ø^ËèK¿Ö€A#5å¿ÚÑMD×J¿Øj¦sG¿á·zö@c¿Ð‡á@!X?AGNBLL3FGL J2009.3-4849PKS 2005-489?ïþ ë©+@?!JƒÔmÑ?%ñEmLU?!JƒÔmè?ïü¬Ë¥âN?S'¬g‹æX?:™¢Ð푠?S'¬g‹æU?ïä¥õÒo«?pU/ø?kZ
-Uê?pU/ø?ïþô¯ýÍ?ýöçÌ9Q? µ#0H?ýöçÌ9…4FGL J2009.9+3544¿æTáé•–?õÀ—Ì:À9«ð©JèÀ;8&1Âð«@ 'ã'ØD@‰éÍ³}?ÑBDþ·«}?ºëÖÂæ˜?ëȆ·>Æ@	eˆšî®?ïÜyGêz]?䪯k"¿æäMÝX‹1¿Ûì{ÿ)ì8¿çgš®lu¿ãÙÎ"7bmAGNbcuB2 2008+35?ïõÙq\"'?Wªölí½9?TMF÷±"?Wªölí½D?ï¼rb…¨N?¥]¢àq O?€ãg^•ìg?¥]¢àq N?î'íÅ:?¢ÔV‰IÃL?­#¬_~±?¢ÔV‰IÃM?ï‰aÅýu\?~g$v}ü?§Ž€¢©/?~g$v}ü4FGL J2010.0+0726?Êß:•ÅˆÀ+}|o½'=À:"ãY×À;Ô¨ÒÁ'@7ŽÆÞ@M˜¤§Ö?ѓ Ì"Â?Ì5¾=gêu?ùZÔG'‡@Ë-´™$T¿ïÿH è?ïòøp¶L¿æðf…p¿é$©'¬¿ïÿëþ@bF?ä"Ä?µwœAGNfsrqTXS 2007+073?ïxè8¸Û}?•¼T-$s§?âøèäU?•¼T-$s§?îØÿl‰Š?±îß­þé‹?¢p	?§gf?±îß­þé‹?çñúªa_Ë?²¡•Ê½L??Ð
«=@j?²¡•Ê½L??í
L	?¦kã!úô?·w‡•ŸG¾?¦kã!úò4FGL J2010.0+7229?¾'*"œÀ@4*Öý¨6ëÀ8Ö§i¦À;пB Ž€@œÞ¬ôd@•ƒb¯É?¥f¦R9³«?º‡[>7Å@Ñ2^!‡@Oø0Ó²o¿Ã¶¨@οâƾ?ì)4¿ã<î
ö¿ä'õÉEY¿ç£S¿šµ¿ìcÝ ÁAGNbll3FGL J2010.3+72284C +72.28?ïök:%Šî?RjÀò³Ã?S)‹´ê$Ó?RjÀò³Ò?ïÎ.
ä$?ŽÃSÞ¢þ?xèúÿí¿?ŽÃSÞ£?ïpŒ‹â?åšëÄ¿?'înŸ£í?åšëľ?ï@LV?ÕG?}©õ(óüb?—öu8W	?}©õ(óüd4FGL J2011.6-1546¿Ûî²Qä©À8°0ã͚RÀ:vJßø#À;Ю2­Ò@ûÒBØl¾@–ž<–‰?΅ ¨×z%?Õkã=|D@²fŸqIï@é^‹P«"?ìÓÀ§$œ—¿æ"Ÿè¿é­Á±ç¿íŒQGpÅ¿ïÿñò÷¿àšÓá*ÕAGNfsrqPKS 2008-159?ïÖ‡¿±Ç?zÆãH.?tù¼ 'Q?zÆãH-?ìW˜+'Ñ?Øùpu…?½C?v£qz?Øùpu…?ìÎm–?£°Üµ;Dô?¹D"Kô?£°Üµ;Dö?êx¤¢§?¨Ø§‡=lÏ?Æmuc‹­?¨Ø§‡=lÏ4FGL J2012.0+4629?éÅ.Ê{Z]@sò«´NÀ7ùvjNRÀ;+ü™C3@щ³¢?þÌÀmBùz?¡ð}^®Ø?¹DŸÂ'­C@±þë-@°fŒQ®?î~Ó-A¿ÙI‰`çK~¿Ý%=ð%—¿ÝæúÀ¥÷÷¿å2Hø"¿â!Ý Y§AGNbll3FGL J2012.0+46297C 2010+4619?ïü;zvå?7'§Pë?>'D,HË?7'§PÓ?ïÕí/5~?"'á¹ä?u	whe@½?"'á¹ä?ï·X0IÈ?"³jqŒÞU?')ø3íŽ-?"³jqŒÞT?ï÷j)|9Ï?Bõ¢ëЦ'?Q+­Œc£?Bõ¢ëЦ+4FGL J2012.2-1646?Þ¦çô™
ãÀ96½ÂmÎ:À9‹¨"ÉX¤À;DŽŒÂÂ@ê¾¥AÃ@¯ï¤h)µ?¼Ì8A(Ù?Øàc¢¼­ñ@³}pn'@	˜JA¿Ç¡QHòã¿ágºú<q ¿éÖæ+B¤¿ìKâV¡Í¿ïÿs+(x¿ï`,Æ1¨AGNbll3FGL J2012.1-1643PMN J2012-1646?ï?š¤5§Ö? ü Áž?˜«yKG? ü ÁžŒ?é*×-Ù R?ÓÔuÕÉ¢?ËT£H™~·?ÓÔuÕÉ¢?éÈ^'Mê?°ìø‹"º—?ÈޅùöÈX?°ìø‹"º—?êÀþ]t?¬›äýyês?Äü‹óº0?¬›äýyês4FGL J2013.0-3717¿åÇFá:&À?‹UX!)EÀ:…Þ\AIvÀ<OÄøÂôÝ@'T-©±@ØIёX?Å6>5è?·æ4|ßN°?ï/_¿_@%;Qå¥â?ï÷5¡L–\¿à—¿9fS¿åÜ=ƒMÕ¿çUr¼Å¿è
g'E?$¿ïüÁr%·AGNbcuAT20G J201248-371941?ïø5ɲ?M}Æ
rÉÖ?O(Û¥5¿¢?M}Æ
rÉÏ?ï÷B³?m1:‡e²¬?Qz™âáù?m1:‡e²¬?ï¯È.'²?€Õ)¼œç?"
ß´["I?€Õ)¼œç?ﲅ碑ý?lì(+›P€?ƒ^"Ú?lì(+›P…4FGL J2014.3-0047¿ÙíXð¾³²À2¿õÆÁÀ9ñÎWçG¢À<l­¨DW@ >eû²hs?ÿ\ÝP¨?¹›ý¢È?™µ ü"?ãcÓCßRá@
±ÇP·?ﶿ¹Sž¿á¦Ç…ò¿à7@=ݱ!¿Ú1Å{`¿æmP›#•¿Ô'xŸ£ô¼AGNbll3FGL J2014.3-0047PMN J2014-0047?ïþsYb?&ev "R?/øÊiÞÞ>?&ev "E?ïý•bM1°?R00lÄw?3Tí–rw]?R00lÄn?ïô9ä›Åk?d7ìç¸?WŒ6Èu(ä?d7ìçÄ?ïô›ØâD?E>ä•ìÝ?VÉàN;{M?E>ä•ìë4FGL J2014.5+0648?͘xU‰'ÏÀ.ï»À:
†¢F†À<MÝÙd‹@!/òù²3?üæÑáÃô?¼"À^ÕMz?¥~ü¤¿?íÀSí"?üÑPÒÖQ0?äÔÀ¡›EÁ?|jâ"pv¿ÕN\¤›«B¿Û'oü'7P¿Ø<EÀÿd$¿Ü‡5^0·ÙAGNbll3FGL J2014.5+0648NVSS J201431+064849?ïå5'):Q?eID˜2'ñ?jÊmÖů?eID˜2'ò?ïð‡Ô õ ?qº9"]0p?^ðW¾À™?qº9"]0o?ïЁö+׋?wiV¸Ñ?w¿ê9û?wiV¸Ô?yÀ?Š'"ø˜m?¥G®Xc÷ê?Š'"ø˜o4FGL J2015.0+1621?æS¿J¦.XÀ$L'ÿK¥À:{gkÀ<™%ÖS^@7Ã¥†·À@!Ì{n5h?·?äq"&Á¿˜Ýèº$dÊ?ã K.Ò{b@5O&óû?ïÿíöé	¿ænyÖ]¿åjŸb0w¿ågÕÒ/]¿Þڌ}ý0Š7{í6OAGNbcu3FGL J2014.9+16234C +16.67?ïì±òTˆ?^èA‹ké?cN
«ówŸ?^èA‹ké&?ïüòBâ?W8}˜???`mèïà§?W8}˜??ï}êpá{Ï?ˆ á1C–?B±ãІ?ˆ á1C–
?ïÃEGÞÖ¤?h/ζ?~]\"®?h/β4FGL J2015.2-0137¿ìWQ
nj‡À3T?Ä;-ÓÀ9+O&®ÀrÀ;¹Z%æC–@ۙC]x@™ä"rÁ?­'w-|?¹;#ÿŒ@}ÔÇm{@êñ#?ïý´'l¤¿Ù妢ì~™¿ãgwÞ]îÉ¿ä§''kþ¿ãå{ð;fÞ¿ìY!¼AGNbll3FGL J2015.2-0138PKS 2012-017?ï%]<EßQ?™ÿ¨?›TXwDÊ?™ÿ©?äÍ|!¥ö?ÓtjÁ@̀?Öe¼µø?ÓtjÁ@̀?ìýÃøWÃ?¥¥1\ëz)?¸à=Aç.?¥¥1\ëz(?æ;ܧ§câ?®t~žÅ?ӈF°±8>?®t~žÅ4FGL J2015.3-1432¿ëèü¦J®&À9›Ø8;À;`þ{›ÑÀ<º­æX@!NoæÂÂ2?ÿÌbäѦP?Ë+¿ 'Å濖HáxÞì"?ÐÀ¢\‹Ç@
°s3©OÅ¿ïà¿]x?ïúkHMw¿åL8½¶¯¿ïÿþó…õ?ïÿü¿ÙŸC¿ïÿý`éNäAGNbll3FGL J2015.3-1431NVSS J201525-143202?ïÿò3Hpì>鋧üVê>ۙo%:å>鋧üQý?ïþ»HN§?P6›2@?'K{…Å?P6›2@?הּÄƅ%?ƒ£·üÑL?"ÒÎÎ^¶Ÿ?ƒ£·üÑJ?ïÿ׊ä>ù¼üq+®>ô:üx
ãL>ù¼üq*<4FGL J2015.4+6556?áaù}øv"@0¤_¿ƒ8.À;tÿ†]À<%ü·v#s@t±ë@ËLÂPr?ßF¿¢AÞÈ?ái¥`!Rá@kÕÓ܌@ˀ"düY¿ïöµ™ª?ïd!È`¿æò
¿ ¼¹¿ê_ ®
ë¿è:´|lb¿ïþ†ܕ˜AGNfsrqS4 2015+65?í¬ZMY‡†?ºUÂVLh?²-•3ÃÏ?ºUÂVLh?ãÜF–‹¨¶?Ó)#½õ?ØGrÒ讕?Ó)#½õ?ê×'úÓ}d?¬'²øº_?Ä£`²
r?¬'²øºa?áø½èÓ?¾-t?Ü"/ÀYâ?¾-t4FGL J2015.5+3710?륛N°7£?óFç_ö	ÝÀ7OE0‹¹À9¼°´hQù@ 5ä¾[@¤H)í?¦~qcß<U?ÆÀtå/D;@"vtÑc5@TÊH8(¿Ü	"(™&¿Þß9K{(•¿áˆ\ZséÝ¿æj>B(¿ë'"ÂÀ'¿ížè]RlAGNFSRQ3FGL J2015.6+3709MG2 J201534+3710?Òµ7Ú¼Œ?ɇgÿԓa?æ¥d¡¹û?ɇgÿԓa?ŸªEaÖÒ?ÓÔøfý0o?ëXn§ŠL?ÓÔøfý0o?Ýy"Cê©?¸œ°Ýìɹ?áC½Þ
«?¸œ°Ýìɹ?£ÍÙ<
>?¡Ü¯Î^?îÃ"l?_<?¡Ü¯Î^4FGL J2016.3-2331?éIˆ½éÛIÀ<†·þ®ûÀ:Ò<!~|À<°¹ßŠ>³@˜¥àyÒÕ?ÿï¤h)µ?ÉÎu™_7?àc·_}>@N1ÿVŒÕ?û[(g¨/ß¿éò^VÍl/¿Ëº!úP¾‰¿Ð2!zÎþ*¿àY	†'¿îZµUů¿âþ@Bæ/AGNbcu1RXS J201604.8-233049?Ñ%€ø5p¾?ÅÜ°¶ò*¼?çm?ƒåG¡?ÅÜ°¶ò*¼?ß¼{:¤4}?ÕHQÌþ?à!Âb­åÁ?ÕHQÌþ?ÅS¹À´kê?´IޘË8Ý?꫏Òå?´IޘË8Û?Øê"o`ÂK?¹#¹U^²?㊵ÈOžÛ?¹#¹U^²4FGL J2016.3-0903¿ï`2jh'–À6÷ƒ8.D·À96œò®3À;ÃÖPM'@²ÐG«<?ý¸¸É	É­?®ØŸ¾Ì®ð?µ«½ž¹þ@ŸIc÷ ]@+3¥Cò?ïó?Ýæzž¿ÚS°àˆ¿ÚsŸŸB%¿àáö?6÷Ž¿ÝåÌ¿çÀÞLQkAGNbll3FGL J2016.4-0905PMN J2016-0903?ïýx¤R¡¸?.±Œ¨åœ?4:ÝjòE¿?.±Œ¨åò?ïúWGl?Z°!$7?F¢ãçšQy?Z°!$7'?ïˌhÀ"?z]šaÉ?z9˟ñ>[?z]šaÆ?ïÖTU†Á`?]mJ‡/yÃ?tÕÕ<ŸO'?]mJ‡/yÈ4FGL J2017.5-4113?Ã4֎ŸÀ@µA•Ì…À:'~Ù#óÀ<yÌí€@ Á-Ý2ö?þ¡™'ƒÒˆ?Á†~Ëb?¶æMý8ûI?ö¹Ö ‹%c@•èO	R?ïŒo_3l>?²Xúm¿Ú|²ÙÀ3¿àÎ1†ŠÉ¿ßÂLì¿äڅ‡"ݘAGNbcu3FGL J2017.6-4110SUMSS J201729-411516?ïý÷àQ
Ò?%ŠìØå¢ú?0@ýw'xz?%ŠìØå¢ú?ïýêŠ4‹4?NrVq,Æ9?0«®[¦a.?NrVq,ÆK?ïïàÈHb?jˉ¹r"?`ë7·žÁ?jˉ¹r"?ïÞx.ŒN‰?YIý"'È.?pÃè¹Ø»Y?YIý"'È*4FGL J2017.5-3753¿î?ï,°ñ™À@E*"8…À;ñ¤óiðÀ<Ö)làÔ@VæÌzm?ý
v
HX?Ôá5"Ç$—?ыt¨H‰?ûLv›gÏó@E¼uÎ.¿Ú?%ðz|?ïïUÑ{¿ÖÝ~`X/l¿áвÀ12þ¿ßݜÞr'˜¿ïÿý¡UûŠAGNbllPKS 2014-380?ïþ'óP¼"?'Ã0ÛÎ"?'ÐÊô=Óû?'Ã0ÛÎ"?ïý‡侍?QR2—l_ð?3ǸÚ"
?QR2—l_ß?A'¨í?"XÉíڑ?‰P¯¶ÄÔ?"XÉíڒ?ïî´ËEHä?R‹l™ág?aK4º·"?R‹l™á]4FGL J2018.5+3852?ÖÎN㏓P?ú¬løQÀ9zeEÔöÀ;Œ 4Rî@ ²þ¤‹:0?ý5¤ãc?À"úˆÇº>?Ò2¿-{@
}ܤ±$Ñ@󟳏%¿è.Ê榓¿éàz~¡Eµ¿½yG'R¿Îk~¾¡æÅ¿ãÊ^'Ӄ ¿ë–BAn	sAGNbcu3FGL J2018.5+3851TXS 2016+386?ê
A)46Â?Áäôÿˆ·C?ÇÊû[/$ø?Áäôÿˆ·C?èv^ÉÂ?Ó£†³g—?Î&"Ø÷â?Ó£†³g—?èN»á¿]?³dđÑ?϶ÅyŠ?³dđÐ?ë!ÿx+"d?ªC×
á0³?ÃxSvu?ªC×
á0³4FGL J2021.9+0629?é¥ÃNëd¬À0Çñ"<:CÀ9Ô¦ló"À<›ûs©E@hþŸ'¼³?ÿ8B·4µ?ÁzØù«Ó?ÃW"üÑÍ=@uîþOý@s''dç?ïùd:<;ð¿ÜÔ¬ÀþZ¿Ú­.â@§e¿Ý•+uϐ¿ç6‡æ鮅¿æ䡟øXlAGNbll3FGL J2021.9+0630PMN J2021+0628?ïãsïW¥þ?s¢Íº"?lŒ¨Z(?s¢Íºƒ?ï՟«¸CC?'"ýœÕ¶J?u0*#Þ^£?'"ýœÕ¶K?ï"1!0Š?ˆzçüI½?Šó¹·³ÝØ?ˆzçüI¹?î"¯ÚH?Œµð•*©??§¾•Ò[q?Œµð•*©?4FGL J2022.0-7224¿ÎëÀ{ÑI#À@H6âëÀ;_~À<½~«Ê@!"˜`©G?ù§»/ìVÖ?Íҟ_+^©?ÊâÙih7?þǧÓï?ûðSå…U¿è"'|É?ïèw'î\j¿â
Lõ|¿Ä›Ï¿Ez³¿åY"‰ê¿ÄãA-qÓAGNbcu3FGL J2022.2-72201RXS J202204.8-722538?ïòqáÈlŸ?W‡"-Ӝ~?[<o&ÀY?W‡"-ӜŒ?ïÇØ'#^U?"c¨•?|ìnPÕ8?"c¨•?ï˜ÅúoÓ?…g4_®o?‰Îd=e?…g4_®o"?îc]¸øwâ?•ãL/Œh?©Ê$pxÉ?•ãL/Œh4FGL J2022.3-4513¿ïéñJ¼Ô¹ÀA;—ædNÀ9•s³VBÀ<þ+êi–@±ß*óH·@+sKQ7*?°šï¯û°»?¹ü¨ ‰Ò@	1eәo¨@§@,ÀÓ?ïö+ÖGŸÒ¿ÔçÃK•U¿áÃ1­÷õp¿ãmOŽ³ŒŠ¿çätôž¢î¿×|0}d/AGNbll3FGL J2022.2-4515PMN J2022-4513?ïüŠ‡"0?6Ay·þ—9?;«Ã_"?6Ay·þ—K?ïûFÆþà?UüŽ
Jn?Bå¼ä|?UüŽ
Jr?ïü7€ÕÄ?ˆ†yß'ۅ?Œ€òʏ@?ˆ†yß'ۃ?ïïSiò?It4O»ì?`¬ãr–.?It4O»ä4FGL J2022.5+7612¿éC¡Éê"Š@5#1;â.^À8éÃ5tVÀ<²<'Î@ÇäX¯™‹@íòœj.r?¤Ò' ½ÿn?¡ñrsï¢?ùÿ¢È"§@oÃgp~?ïÏ"‡"‰¿àâ¢Â7G•¿ä»dàTi¿âA3¦ö¿åÍ·þßn¿åòGAGNbll3FGL J2022.5+7612S5 2023+760?ïúĸ~*?CŽÜ
êŒ?DíWæå?CŽÜ
êt?ïøâîC")?c³"»œxü?LtFñïWµ?c³"»œxý?ïåäÙªþP?o[õd<ø(?j&U¯?o[õd<ø.?ïó_yÛ¿ª?I Ã3¶'?YAH€­??I Ã3¶'$4FGL J2023.2+3153¿äþŸvnNõÀ½gý?[`À9¡ §?tŠÀ;oÆÐ3‰š@!]´8×7	@qú[{PÙ?¾lðï÷ä?¤R×¾Bph?ênwÂYV^@lF__áè?Ö£e_Ö)m?ï±ß`£-í¿Ù¢'ÌM¡¿âç!A™'"¿Û؜cÎ[˜¿á‹ºžLèAGNbcu3FGL J2023.2+31544C +31.56?ï®ò'gL?ƒÃ°°ÿn?"{C_f-G?ƒÃ°°ÿl?ïã¯<`Ž?•r‰}^^¢?lPÃbŸpu?•r‰}^^¡?î÷¿Øïûe?šAÓ ('? "qI§?šAÓ ()?î–ö"Ûý–?–sòmîí¦?¦Ò@&?–sòmîí¦4FGL J2023.4+4127¿çò}ú%vØ@Õü¦¯+ÒÀ8ÿÊñ*z'À:ÕKoj'@ wýFKê@Œ~»ÇÁË?Áõ…Rº·÷?Ä·Xtû@B"~ea@wóòUk¿ïÿôa¼2¡?ïÿ
ÂPÇï¿×£aÔÜ;¿â(orŒ¿èќªÆÈ¿Ý#®ÆQˆ‰AGNbcu3FGL J2023.5+4126SSTSL2 J202336.19+412527.0?ÞeêücÞ?Ð%Hªˇ?àÍ|ŠÎ?Ð%Hªˇ?Þ3ìðÁ^?Ø>ÄàS‹?àæ	‡þŸQ?Ø>ÄàS‹?忦¼‡?º³8½Ü?Ԁ²‡çøó?º³8½Ü?æþí©?½ËMSØü?ÓÂÆ%Ö­?½ËMSØü4FGL J2023.6-1139?×vSÊñÀ9­Ð¦v ïÀ9Y´Ñ-"žÀ;õSì^ó@w#Ñ@yî?ÿc<Ù¥"?¯·Úø3­×?À­aw"6-@ã9:´0õ@
w헝•þ?ïÿ¦n£¿½eøØCx{¿â<XuâÛ¿à¹_²˜¿åë'H'@	¿í'¦ïnAGNfsrq3FGL J2023.6-1139PMN J2023-1140?ïèQ±1˜?k¯uóšGh?g®NôÎgá?k¯uóšGn?ïxm:'–|?¤ÀëܓË4?òX­­0d?¤ÀëܓË4?î§JÌÑÂH?›ì¾&9ï?¥‹S2ãۃ?›ì¾&9ì?íëåA€žY?'€à*Ï?° Õóû
=?'€à*Ï4FGL J2023.6-0123?É]Ȓž@mÀ5þ÷ÂDÀ:[§ŠóäÀ<U›ÍP€K@ÁË[ˆ'ß@Íp`»?ÂeãØ×ó?ם 6×,¢@ÏÄ~I±û@ù(uj?ïöŸ>I;Þ¿ÓG>'òŽ¿Þh3Æ)ñ¿â¡ÎAÒ¿î@;#Â|è¿ÕS"g*±"AGNbcuPMN J2023-0123?žPÍ Çq?—@ó.k?ï
ɒùÅ?—@ó.j?ØÉã–3?Ô!ˆ¹ž®?ãÿ4÷g?Ô!ˆ¹ž®?¥ER		fZ?–Ûþíb/3?ßoiš?–Ûþíb/3?ãg{Q^?²†4)k?ØÅÁ1	]E?²†4)l4FGL J2023.8-4828?åã?{ÈÀAz»˜Çâ'À;L-ê
ËÀ<°ìˆ3@@CÁNêHß?ÿû©Y*=Á?ÑØ
¢gÉ?±ÉòQì†Ñ?Úµò€:¢é?ÿ·	Øi
?ê0‰jwm¿ï5§¡ïÿW?ÝÊ3)ø÷οÜĄ¿Aô¿ïþÍ?äF'?ïõ@‰]tAGNbllPMN J2023-4826?ïý)@Öo?=ʵƠVV?6µùOä?=ʵƠVT?ïõ>é?{Å]uÒ³?Uÿƒâ-ä¾?{Å]uÒµ?ï£þÍC¯?…Ì 5Îíà?‡L¯7ç?…Ì 5Îíß?ïäjNç€@?b3ž"¡?k•±¾Ä?b3ž"›4FGL J2024.4-0847¿áŽU¯­À8¥"¦óõ0À9Ë,´"ðãÀ<#:Š?‰ƒ@ £Y5ü?ÿ!{zÊ¡y?¹×Ó2Ó?ªñÆ+rõk?ñˆڀ·@ùyŠ˜?íbfâ(r¿Ùuã'¥¿âg…_ÐË	¿Ü%l 9±R¿Ü
EbàŸè¿è©rÀü¨AGNbll3FGL J2024.4-08481RXS J202428.9-084810?ïôZ"=?Qr<Õaq®?WÉÿK»ˆû?Qr<Õaq¬?ïûàŒ@ZS?X]Áb®	7?@}Îþ–´R?X]Áb®	9?ïÞ½á'6?t(FN×~?p¡q¶åX?t(FNׂ?ï­s_pE?mõøÏqi?"£>è#îÝ?mõøÏqi4FGL J2024.6-3252¿ï™?ðÀ@rö@c^À9[ù‹q¸ªÀ<YhQ"2@'ÝžVAÖ@хÞz?²#Š•š±?Ã}ƒa@êÿÓ>×@¸	™¿Ø¢PA¶Ù›¿ß	Û !³"¿çqž]£Ÿ,¿æªõwÖ¿é¼]°	s¿ïÿ³©æ÷AGNfsrq3FGL J2024.4-3254PKS 2021-330?ïøÕøQ?L+:Šªè?L¨þ»ü`?L+:Šªã?ïú[¾S^'?[!Æ_'l?F'²…ºë?[!Æ_'k?ïeËÄW‰?ˆ‰Tä'?"\‡uÑ?ˆ‰Tä'?ïñyñÃÙ?L>ÌRl;?]
üxM[?L>ÌRl54FGL J2024.7-2328?Á'¨MÆÏÀ>Rk?éúÛÀ:¿ìMøÀ<€¾‰¬½@o¯YIre?ÿ3-Ú-Þ`?ÉõDæf?ʬ¬è*÷@&ûëýê@ÓÊJ¼?ëM¾,0
?ï]ËB83¿â›6A°y…¿ÜÊ®DK‰k¿å5¯¿ ¿S¿ïÿý¡UûŠAGNbcu3FGL J2024.8-2331NVSS J202442-232826?ïîI?aûEԔ^?ab¶÷èð«?aûEԔb?ïáܲ"ã?'ÌöI3×)?n#M{à?'ÌöI3×)?ï~=4œÝ?‹4‡ä³2?8Y}ìdz?‹4‡ä³=?îî4|Æ¡0?ŠšÝ…dŠý?¡¸3•í?ŠšÝ…dŠý4FGL J2024.8-6459¿ßLòšy]3ÀA'žÓ•>À:ˆ¨½ùË3À<†\S½í6@%ÄRTá"@(\ÅÓ´?¼øӐá9@?£cV9?äÄ°¾Ï3/@ÅÛAÖ?ïý@h¿Ûšðü××m¿é6ù5¿ã‡!A™'"¿ãmÝô<}_¿éMOõ^fAGNbcuPMN J2024-6458?ïþŽäDªÉ?$3â€78?'»µSc?$3â€7É?ïþoþ¾á'?DøšÀ³;?)퐥?DøšÀ³G?ïÔgì^<Q?vå½I`'?uÌ	Ðáן?vå½I`"?ïþòó|?†dδ? ÐÏø?‹É?†dÎO4FGL J2025.2+0317¿ïúýÏÏ8½À3`4óþÀ9:yÂc½?À<®Bž
B@gÑØÐ;A@†ÛPô?®h¼ày/Ÿ?³‹ÉLd²‡@çÖs>»ý@«é¯¼'¿ÜFï}¦ÉÙ¿ßða<æ¿ã«DAM}6¿ß¥Iû÷‡¶¿çnÅ°xÙ¿èç(bõ˜žAGNfsrqPKS 2022+031?ïþå	7?lÓÄÿÙ?!¯oœ
Ô?lÓÄq?ïü«.ò|?Yý¦(ù?:¦ˆo,4?Yý¦(ð?ïÚãíEø?wÏ9(–?rž.	]ú?wÏ9(–?ïüªØ¯ºÀ?-:G«êþ¤?:©:'*'?-:G«êþX4FGL J2025.3-2231¿êBŒÜ'À>"ÓÍ$áÀ:‹Ú¨W¢À<nU•]ʶ@ '6Ö*ïm?ýégØVmË?À¦´_B°ª?±Ìö%‹«?óá3ÁÎl	?ù»fØ&G?ï÷ڂû¿ÜªWA…[t¿Ý¯ïüý—¿ÑÙ÷¢äF¿èíòKâV¢¿|>ûq-AGNbcuNVSS J202515-223016?ïè':.%?dÑøfgÁ?gØÅÑÚæ?dÑøfg¿?羚\‰'?—¦Ä¸H"?†T(ú]›¥?—¦Ä¸H"?ï]÷OÂ:?ųyjk?"A¸¼b?ųyjl?íùl`Ù%?"êE{¢Ï?°4œù6×0?"êE{¢Î4FGL J2025.3+3341¿ä•ÔZÁmÑÀR

ù¾À8A=e¼{À:™-BŠ¿@‡/›#1ˆ@Ò±-4±?²jî «†?ÆÖhA‡ß³@s ÔƖ@ÉÃØÝQ?ïÎxžwNì¿å«ã‰o€¿çý"såªê¿ç8?!(οï-ád´`¿Æƒ~_pAGNbll3FGL J2025.2+3340B2 2023+33?ïcY'9?›õS"é¦?""ͽXÞD?›õS"é¥?í{€iO?Èùt!4»?´'Cüµ€?Èùt!4»?æ‰Îè^Œ+?³k¢óé°ò?Òìb/Bç¨?³k¢óé°ñ?끻C)Ž*?¬¶ñd<³?ÁùóYÇ[?¬¶ñd<³4FGL J2025.6-0735?æ\©»°o+À8cY§TmÀ7"§&J¥À;;A¼bò>@t‹gÒ¢$@ƒÅ_AË?Žµë`ðR?¸ÝÊ @&sü"$íö@ Bî «†¿Ð7X[á¨&¿à9RÂÀp¿ä¸;æ`Ê¿åýÉÄڐ¿è½jęød¿ëS/uKAGNfsrq3FGL J2025.6-0736PKS 2023-07?ïêyóAÝ?aRŸU?eû†¾"è?aRŸUŽ?ï×Y¡L?"¶è·$‰?~4Sr/Y¸?"¶è·$Š?ï¹ØYeS˜?'=É'}Üå?‰é¦«ö?'=É'}Üä?ïäð8Ø*J?d©ß@¹U?kÇ'Õ¶?d©ß@¹S4FGL J2026.0-2845¿Ö7ú*õÀ@"ƒ‡ß]À:˜i6$;À<Míض@HLó"Ìß@dqcðja?͘+ˆy?ŜÆʪ2Ä?ö–•ˆ'á@	Þ'h#ֿ湓¿ºëy¿âÇ`Ƥj¿èýب£!Ù¿è"u'À²¿è¼ÕÞÄF¿ïÿ½ÅGóAGNfsrq1FGL J2025.9-2852PMN J2025-2845?ïûöb^Þ?@—Vó¸Ák?@'®v"Œt?@—Vó¸Áv?ïý´ÞfV
?P.!ò!tu?2YÍO³‡?P.!ò!tz?ïs¥£Ó,:?‰$O{1ËC?'‹K…šx¾?‰$O{1Ë@?ïó'\Þ\s?I@—–â³?Y±FCGg?I@—–âÃ4FGL J2026.1+7645¿ïü¸T'ë>@59>ê ›À;
æ_E	õÀ<«­	¸æf@"Š[Ö?'<?ø›%:L,(?ǝ¤ÖŽ—ˆ?ÆWe—‰t@‡ÿÞr¿@T=ïϱ¿ïëUN.K¿ï×ßàzԈ?ïå³vQì?Âv'^¿à´€€G¿¾³ÌÓ¯ëAGNbcu3FGL J2026.3+76442MASS J20263126+7644487?ïú-°¿ç?CùÅÔ[¯¸?GI=cç?CùÅÔ[¯Ë?ïø%¢†H?hß֖F§?OiwÍæݽ?hß֖F¦?p‡v–Ã?}í`ÎíÙÝ?€›Þ"ZO5?}í`ÎíÙÖ?ïÄ¡®wÜ?pKÊ*±C?}¯1(ÄÄ?pKÊ*±C4FGL J2026.6+3449?×͍¹â¿ÿu
xŽ‡À9¢ZÐ0.œÀ;?Ö§A"	@ s¹£¥60@CÂÍoŠ?Â8Éu)wÉ?£ùÉÁ:ف?âUKÚt?ý3ßJӸϿîÓAáKßÒ?îj»_¼þù¿è`¼mÙø.¿Þû]Ay¿ã–,A§j=¿ç¡®pÁ3<AGNbcuNVSS J202638+345022?ïu(Œ9 ?Ë&¼4?'_ZîxÛà?Ë&¼4?íá"ç"ðm?ŗTq¸Õ¥?°öèÃØ|š?ŗTq¸Õ¥?í쨞XÃ?¢ù̂ì	g?°Ÿr»
9ö?¢ù̂ì	g?ì}'L_È?«Ä¸Ó¬
?¼m¿õ?«Ä¸Ó¬
4FGL J2029.1-1839?æ®OdߙÀ=£·•-#OÀ:°dPâp£À<kَ|/&@ˆ>	P
Ú@ÙaÃiv¼?Íe˜¶×í?Ó@ª; g@EQÄ?ÿc‡ÁÕÍÒ?ïßÓ™hF¿Õú,@ûÆ¿äTž›·¿åÿ`h¤
¿åU'ÿùJ¿ïÿqšw+AGNbcu1FGL J2029.0-1840NVSS J202900-183709?ï{¢Å5?ŽÄìⓏ}?‹­íçY2?ŽÄìⓏ{?îՆC&]?­%–ó2¾?¢§›Í–ú<?­%–ó2½?ë©È§Çâ3?ª	¡úéÉ÷?ÁXÝ`àw1?ª	¡úéÉö?êW,î
»?§î×¥ªl?Å£LGÉ?§î×¥ªk4FGL J2029.5+4925?†øN€ö6@]wúã`À9õ6À;jÍë°½£@´Øö¦ºê@×R9ˆ·Ê?¶ÌMöØäÞ?ÓA­§m˜@ÙgÊêt~@ó,ª-®?è$ÁUuR¿É/¥ßøù|¿áÓ+UïÞ¿èì›Sþ¿ëF–½FG¿ïø3þ_AAGNbll3FGL J2029.4+4923MG4 J202932+4925?ãj§BJx?ÈYyYq¾i?Ù*±{kÚ?ÈYyYq¾i?ï¡æ}÷ß?¡Îv‰¥í?‡†`'8ˆw?¡Îv‰¥í?ސ?mÐÿ?º[NrÓÐ?à·àI€w?º[NrÓÐ?îìSK:f_?‡¼
ž¤vR?¡:ËLYš?‡¼
ž¤vR4FGL J2030.2-0620?á{sâi8åÀ8Ö®::ŽqÀ:GÖ(ôìÀ<%o•º@ǯïœZ"@qƜ1#Ž?º…࿝å.¿¨>,œ§QN?êG±ÚØÿ
@C×n;qñ?æ*K-$ü9¿à
è`ܺ¿é·<­/x"¿ÜÞ>ÄáÆÚ¿êˆe>É…¿Ä5»"ÖCÄAGNfsrq3FGL J2030.2-0622TXS 2027-065?ïù?…ê–œ?K㙗!¦1?KèU¥'$?K㙗!¦?ïþÐ#X}??¿ùâlí/?"þ­Êx2©??¿ùâlíb?ïÄuý?c¿w9ÀÚ?}ô~Å7'i?c¿w9ÀÚ?ïÿX@)Eõ?D¡Ò–o´?÷ú×A]—?D¡Ò–oÆ4FGL J2030.4-0502¿åù*€owÀ8Lma,jÂÀ;,,"ÜÁ7À<ƒØÐç
Á@ ZÑÜV,²?ÿ•;fœ?Ñw'w?«)ˆ9ŸÞØ?áj‡þf¢Ì@'šËrړ¿Çӈé:x¿ìxþžÖð<¿áÿ®ÁžñG¿à
ïAkÛ¿Öµ»€Ê¿á·1$e:AGNfsrqTXS 2027-052?ïÿYnðº?
§ÔF<@Z?Ür!èÃ|?
§ÔF<@Q?ïþªû«èY?H"U(?%PEAzyý?H"U?ïø—^R?^<ӝÅJ?M¢†·—Êž?^<ӝÅU?ïüO"A<?-öⳜù?=‡sÝö!-?-öⳜ²4FGL J2030.5-1439?Ün\¤RÀ<o"}cÀ:¶Fà‡•À<yŒ†‹ŸÜ@ çþ¥aùÅ?ý©•?ÇR¡ãj?žŸyzÀ;?Øß#¦@@víb£æ?å•6Þcx¿è»îQ"ñ¿àÍ,¾¤ëݿׄH"S6^¿ÏU-Ä^iB¿ÕC¿ÝÑAGNfsrq3FGL J2030.5-1439NVSS J203028-143918?ïü˟Wt8?/õüF"æ<?9£D^AÅ?/õüF"å·?ïþ:uӀw?JÛý͹µÚ?,X¢Çøt?JÛý͹µà?ïøhšðÒ?SsÎÄÙ?N]—ø<¹7?SsÎÄÞ?ï÷TOë
7??ø%ëç-?QW`)咂??ø%ëç@4FGL J2030.8-6959¿ÑË2I»("À@ç]þ¸Ø#À;¨mqóbÀ<²˜§+R"@WR
é͏@ځNš?̧ jْ®?²ú2¡ì?äyºHeÊ@ßËZ'œ?íqD îÍ~¿ìKIt¾þ¿ÅCŽõü›ò¿ç.ðäJ7¿ÜEva†,Õ¿âg¡yâÅAGNbcuPKS 2024-701?ïü¼ùàºf?6˜gÄ?:0ú,ؕ?6˜gÍ?ïþ'H¨NJ?Bþ!0Õ?'Ûu{`¾?Bþ!0É?ïÛÅ^©_?v¶,¿éÆ{?rP«PuÎ?v¶,¿éÆ?ïô;ZD?DWGKgÅs?W‰õKwÆÞ?DWGKgń4FGL J2030.9-1621¿îÌiïá#¬À=0]¥qÀ:®p¦[HüÀ<~b¼ºh@]µ%ç@…	Œ³?ÅÛï?z?£ö AÏ?à_‰gó.`@œ¤MQ¿ì0Ï«¤¿Ú6à;êfç¿åyÄ6%¿×'@~b¿×.ž
œ µ¿ïÿ"Év7AGNbcuNVSS J203048-162224?ïüxÿ¬K©?3JùÜËÄ?<8¢¼?3JùÜËá?ïþdY«üÞ?CãȹšEÚ?)ºe@2'×?CãȹšEï?ïèF^ßMq?n$6a©ñr?g¹¡ ²V?n$6a©ñ^?ïõMë`ç?FÅr袻¸?Ud)>1ñZ?FÅr袻É4FGL J2030.9+1935?êW•8íÀ'
"cØ­À9¢^)ÊÀ;î=ÚV"L@å4!Å£?úpŸM7Á?·›þ£´{?Ä,ÞÅÈ¡š@°iS@/ÅÇ
â¿Ù4åOz'—¿ÚF0ÑY#ˆ¿ÖCÆ=çl5¿Ï;>š@¿äŒÄŸâ¿Þ|Û·Ì5AGNbll3FGL J2031.0+1937RX J2030.8+1935?ïàÓ3X%'?i·%¨É—½?o,̧Ún`?i·%¨É—º?ïâFš_éG?‡ÙFy8Ô{?m¹e ¸ú?‡ÙFy8Ôz?ï1ÄTÁo?™¯'0S¬?Ÿ9ÇugÒ?™¯'0S¬?ïWh'&ƒ?€I~͐xÏ?•òí»/Å?€I~͐xÏ4FGL J2031.1-2615?Úoh£ôÀ@G¦a(9À:‡îúôþDÀ<Â*²[1@ÀJˆdh@&†|†c?ÄZQDÁ%$?χ>.@bϾÔã?ù²jÉ!œˆ¿ïÿ"=ßßy?ïÿþ½à ¿¿Ü‹©_>¿çN(Ÿ~¶¿ãf[)òB¿äGGQÎ(íAGNbcuTXS 2028-264?î†ÉTwíÏ?ª°,![¦?§"j¸#?ª°,![§?ëÅ*nöR?Ç­Œ˜;Œù?ÀëVD&·©?Ç­Œ˜;Œù?éó&Z¼;?°àqG
µ?È3f•£?°àqG
´?ål®€ìú?¶OÍ7¢e?Õ&£Øþ&?¶OÍ7¢e4FGL J2031.2-4121¿½øooþ¦'ÀAÕ¥~ª*À;.¦Üx;À<³JÖ½ç@m·&tU@?e¦MC?ÎÖþÎ?à­]€ä–î@
¼{F@¿òRBm
¿îCšžý0Ã?ïÿÏù§÷*¿Ü/#" ¿æìÎÊÓοîCÐàWÄ¿ïÿ–ƒd£ïAGNbcuSUMSS J203056-411906?ïÃÓ*;E?‡A/Ž¼¯ë?~xjâ]>?‡A/Ž¼¯ë?ïûs¶Õºƒ?[Q Må?B1$©õÖ?[Q Mî?ç³ÚJ£(?²DP~¦ë?ИKj¹¯?²DP~¦ì?ïíȺ´	q?X°Èá¢?b7EKö9?X°Èá¥4FGL J2031.8+1619¿ï¶¥¥'À+ÿŠ:›À:ºZ/ ~üÀ<?Ô|ñÃ@ó2Ûõ^¼@P³''d?É1Á¿"?½ä<Uäˆ?õ^yLò÷Ú@&¢¬ì?ïþÔI˜Ð¿å.)ÿ,ñP¿ìgß?–ÀÓD`,;¿í©¿Ãyè¿ïý›l°ÚAGNbcuMG1 J203139+1622?ïûû´?K³Co6#?CóÇÜ.¦?K³Co61?ïﯛ)»?|L2^
ø­?`PdùÖD+?|L2^
ø±?jÁ£?‰JùnñHQ?‹å{ϗ?‰JùnñHO?ﺹŠë:­?rɇÈVàK?QE1Tõ?rɇÈVàP4FGL J2032.0+1219?íq2ãÎäÀ/"š8ûÊÀ9ÃÁc>ÓÀ;ä"Àìĺ@)*Û£@ž®"i›?ÀCŸ¼ô<¨?Àìõ·&È?þ]†Þ«òb@Ç
ÈÀx¬¿±	[]ô§Ý¿åcØ·¼šP¿åʆÁ¥§D¿äG-»úír¿æ¬L#Å&¿ðAGNbll3FGL J2031.8+1223PKS 2029+121?ï÷0˜;ӗ?P'f݃ª–?QžÏˆXÒ¹?P'f݃ªŸ?ïü«0°®I?TÏ?¯3;N?:¦zz¼R?TÏ?¯3;M?ï¸ÙmJV‹?K¼0N4Ü?É¤­j]?K¼0N4×?ï⠊©é³?X"x•TØÂ?m_uVLÑ?X"x•TØÄ4FGL J2033.7+6308¿ç:ß­ðN@*øœýç!À;CÛ÷âûÀ<—έwœð@!'x´FÄ?ûÚ®‡ggî?Ì£J(î?Û@=²¾@ˑcj2¤@›KutK¿ïþ³™õßì¿í¯>;¤ò?ïÿÿ^ðP`¿§œÅ+	¿ßŽý'¬¿ì9Z'}rAGNbcu3FGL J2033.6+630987GB 203249.5+625814?ï¬ùîäCô?'2Ìlx5?"Á"Fï1?'2Ìlx5?ïÁ­kyÜN?–¦)ž¦Å?)JCØë?–¦)ž¦Å ?í\rЦ5?¦4&MÃe?µizÎWç?¦4&MÃe?íؙÀF"? Ljß;×6?±;1ýÎï¦? Ljß;×64FGL J2034.6+1154?íS_ÞWVÀ0Œ¬¯öÓ1À9YiÂ;ySÀ;Žpð›@r¨h3@ÔdcP?½-—ÿÜÅ?Á¶—;?þi¾Å£à@k–JYÀf?ä"ÝÛ
¿ÝÆG·J/¿ægfÁ€Š¿èFl*˅¥¿è'áý¶z¿æXøŠ.ÃAGNfsrq3FGL J2034.3+1155TXS 2032+117?ïÕ¬Ýìýq?Yû‹ µ?u)'	Fì?Yû‹ µ?ïý+kjY®?Kþ×Åý?6¤¤­2?Kþ×Åä?ï2Õš[Á?'"}eµæ?™¥^´‡Ø?'"}eµã?ïÓÞòíŽj?cDªӃ‡?v†‰8Êù?cDªӃƒ4FGL J2034.8-4200?á« _EtÀB3´ÃÁ‹PÀ:C¿šµ"ŒÀ<a,"¹º@ W$"2LX?üsAü#Òm?Á¬ÐB£¿?ÁŒ÷Ÿ´:Û@ô즆çæ@db̨å'?ïþ6Ò$$¢¿ä杞6€¿ß¿YFÃ2ð¿ÎxÕäÎv¿â'jeÏg²¿äìf€<¦OAGNbll3FGL J2034.6-42022MASS J20345108-4200386?ïþð¥Šeþ? #0ù.[? õ§Y ? #0ù.p?ïý¼]`?P
‰ÈŸ=?2…m5?P
‰ÈŸ=?ïðˆ=Q"Ú?gÜX¢Ü¶ã?^ï…\öM$?gÜX¢Ü¶ñ?ïәP£é‡?aK—ë
r?v3W®<¾?aK—ë
{4FGL J2034.9-0450¿ï㷊oó•À91öº «À:tBúP"–À<N¿ïn¸D@T¢Ëò\S@b¥Z'"?Æ!Ô¦Šî±?Âþl©±?úÆqÔX²I@Mq6Ô¨¿êá:­z÷î?ïö'÷䨌¿äSÓâ?Ð¥¿äÈ'­ÄÊ¿ãÏ >ŽÛû¿ïø²<'ÎAGNbcuNVSS J203508-045029?ïÝÑúo'ã?sxÁ&€Å?qÈ7n?sxÁ&€¾?ïëGþ?…˜A÷?d÷é¸sß?…˜Aù?ïPÐÏ¡T?'°&ÒÐ4?•åæÕ|¥?'°&ÒÐ1?ïpmÐ[?tKb•a?'ò_-åôl?tKb•a4FGL J2035.4+1056?ڊQO‹p½À1>F{åS¬À7²¼MùˆÀ;4Oó]Z@zø?kQ@".:¥î<?—³®e%0?¿¦Û ¢ŒÝ@"'o°'@}4JµZë¿Ë kÅËÑ¥¿â%¦V]Û¿å<Z#bØ¿æ£Pg  ‰¿ê$¯â±;¿èæÖcNƒòAGNfsrq3FGL J2035.3+1055PKS 2032+107?ï¾~Hû?Êòò¹.#?€`múA:É?Êòò¹.'?ïÚ雧‰º?˜‹'}ηp?r‹2,;"ÿ?˜‹'}ηq?Så?Š³àæd:°?]9뜎?Š³àæd:²?ïø¦'±è?DO¼†Žp}?MeõÁ8b?DO¼†Žpl4FGL J2035.9+4901?ӝ¾Â1&V@ë@UZ¥À9‹'ªhô¶À;¸‹C•@ Ɋ8þyB?þŒÜò´½â?¼eáÜ(Šc?¼ØüŸ½?þ‰Às"6Œ@­¸ºÇË¿ïòö—¡qÕ?ïýŠuV¿âé>›A:¿ÒXÚaµÒŠ¿ã€¡{k¿Û‹ÃîúAGNbcu3FGL J2035.8+49022MASS J20355146+4901490?ïô©«æ?^¦'P+¡?W̭Ĩ3e?^¦'P+¢?ï¾Kѝ¿`?—‡%©Pæ?€m˜(?—‡%©Pæ?ïz#{aÀ?½š¢YU?»ŸP"Çè?½š¢YT?ò…\;?"¨'0imâ?¥D ×ª<??"¨'0imâ4FGL J2036.4+6553?ï¾¾Qýß©@-—µÐ1\À9ûžs.À<(Ød°ƒÁ@㬁u`?þº}>ïÿØ?¶_adsòì?ÃÅ£e@	Ê*[]@
,™­æƒ?ïþ;¤ñ¼p¿ÌcÂÈ&C¿Öë÷öFC¿Úå»d°¿çÃâB׿äLD琝rAGNbll3FGL J2036.4+655187GB 203539.4+654245?ïúV:Hká?I›#*ä¦?F§ÞPxâ?I›#*ä?ï๰§?'–_+ù/?oFâOXp?'–_+ù/'?ï¨]r?"۔ÚÚ?…è¾x£xå?"۔ÚØ?ïìö:G?®lqPÙ?œ'~á8·?®lqPÙ4FGL J2036.9-3329¿ïxÁ†LàÈÀAśý÷èÀ:^x]ï"À<H™¤T(@!$/_>)?óŒïœÛmz?Ð.è¶7_?ÏÏ{¨Â×V?û'ÿ·@¨éÜ?Ž¨ºH棹¿è)!ACAH¿äLXÓÖ¬J¿ÃÃ7Îxt¿Ê/ÁŽ«)¿Ú&èa¨¼wAGNbll3FGL J2036.6-33251RXS J203650.9-332817?ïêÑM9YÛ?aåˆØÕ^?e.²Æ¦$\?aåˆØÕ^?ïý³¥ÇÝ?FÖ§?ô?2bӑÁ^?FÖ§@?î¨ç¢J?šmåZ›Yñ?¥хÛ_#?šmåZ›Yñ?ïõ§ßs!o?GT,7Rz†?T°A½"?GT,7Rz€4FGL J2037.9-0504¿ïéÙÊ |2À9ñD»ó¡À:ý]0\¿À<‹;Óåj@ J@–H+?ûGã>(Y»?Ô2本ž"?Ìÿ9[–S¿?ûTâæÅ°?ý?]Rìa?ãc	¼Ad¿ëI‡î'ð¿Ï1~¨&¥¿Ü&š¢þ¿Óôk0Ñ¿ïü>àŸ°AGNbcuPMN J2037-0508?ïöú	Vä?PŸ£&Þ&*?RíËR9^?PŸ£&Þ&7?ïùªSHç?uª÷åOí?K­V²Üa"?uª÷åOë?ïÒª×?…S>Ê®†?Œ{Õ{ÊE?…S>Ê®ˆ?î҇?y¦ÿ‹Ë¸®?܄K^B?y¦ÿ‹Ë¸«4FGL J2038.7+5117?å"`*±m@ÿA<á1ßÀ9g{o'VÀ;A_ˆü"d@¦ºZ•@Ó}c-Ø?ÀúX R…ß?Ó±Zÿ@¾6`]'@ˆ"ŽJ[¿â°¿?ñ\¤¿Ûò–Šñ`*¿äÀ~«Ê*¿èÝ_ìú•¿î¿ñQçSa¿ïÿW-ä>ÙAGNfsrq3FGL J2038.8+51133C 418?믜ð£L&?·Ÿ9îm*S?ÁAŒ=rÏh?·Ÿ9îm*S?ïޖ•w£?‡†¢"ã(Ø?p´þµD.–?‡†¢"ã(Ú?â½wÐ{n?·.Á"Ö2?څÁ_	&?·.Á"Ö2?ïgµê˜?€¬Fà4é<?"Ž	B­?€¬Fà4é:4FGL J2039.0-1046¿çzPœÇÉÍÀ<¼{՝VÀ8¹
…"ÿ×À;°¿òɶ˜@´VØ~ܪ?ÿK Íj~?¦I³RR]E?·Ûþ2¡N@÷•p?-<@ٔ媿1¿Õ§D}"¿×ÖÈ#DӚ¿á8ãv\~¿àÓ> L%È¿ã¾XˆWR¿èM3>ñ­WAGNbll3FGL J2039.0-1047TXS 2036-109?ïô3."cê?T#½žØ,?W™¢×8)‡?T#½žØ&?ïÜ'0T?'®Ýγ?qý7qgÖs?'®Ýγ?ïSbdð«?"öB±º¿?•"¼SaêÔ?"öB±ºÁ?ï!µà?"ËÅñÛ:T?žûß=éCç?"ËÅñÛ:U4FGL J2039.3+2150¿çÍÉ!|À'©K{(•JÀ:"Ï$•á~À<CN"¸‰@z…Nˆú@ºòDUšf?Í»Ûۈ|?хRdÑ»Ê@ø¸BÒ¨@'ہÆi?ïÿEÅÜèìêÿ½ºá¿áiž)KS¿ë¶
éh¿ïö¦…:g¿ì8ÄL0ZAGNbcuTXS 2037+216?ïñ®†¡Í\?j‡,L¸?\¢ò¼eG¼?j‡,L»?îñËuö?¶=ÇMGÐò? ãH¯ –ù?¶=ÇMGÐò?ìÃo?j?¤êÕ{4Žß?¹ä†o°?¤êÕ{4Žß?íÓàÏè‹?"á!Ü¥?±`ù‡`»¬?"á!Ü¥4FGL J2039.5+5218¿Ãà¦Ò4@[]ô§ÝÀ9èê1ÄÀ<Þ7X@!ž†)þ?üÃPíX]?¹&+¸À{[?¨ˆÝ³N÷?ðcª2n?þ!M:ƒ?ït²ÄãÊ?¿ïüáù?ïöóçÃɿ丕k7¿Øædÿ´¿Ô…qÄhzAGNbll3FGL J2039.5+52171ES 2037+521?ï7èM?W³ÕÖt©?a[Oȳ9?W³ÕÖt¬?ï³{‰"¡?¢@Œ½?ƒ!·y×Ð?¢@Œ½?s!?†…Ý.e?‹Z#;ÿ÷·?†…Ý.f?îƒÚð3?£6šÚU×Ì?¯×ÏPüã?£6šÚU×Ì4FGL J2040.0-5737?î‡z‰cGQÀB‡DÃ~orÀ:+jî‹cvÀ<K¥"cØ@mdõxµ@ÉÚª"?ºYF¾U?¢Ì~HZaË?è¢FçE?õ´k×êb4?ï˜Úϐ¿áƒ]©~i¿æJÀ¾¡'¿à¶}Õî´~¿éâ…0V	!¿ïôÚgÀºAGNbcu3FGL J2040.0-5734PKS 2036-577?梁òÙI?†ïªÓ"çÀ?†'`I­'?†ïªÓ"çÀ?íñy0)cb?¿î½¾«?°t6~´äö?¿î½¾ª?îâ:¾¯‡ž?"å^v¹Ã9?¡ÜT†?"å^v¹Ã7?ꔬKŸ¥"?®âmÅý?Å­Nсku?®âmÅý4FGL J2040.1-4621¿ÓñiBÌ7ÂÀBкs-õÀ:¶€À<p.½'¬î@ øŠ/nW¡?ùâؼ²£?Å®_¹Îî:?Á¬;ç%?ýõÇèa}É?þ1ÿ§?êØ+ÛPO¿ï痞—°5?îõ«þO¿Ù˜*™0¾¿à/ ×{|x¿Çyœ#6»ÔAGNbcu2MASS J20400660-4620180?ïõ¸Pœ0&?PE效#d?T^ǟ±‡?PE效#h?ïó`Ù·Ù?€ŒT?žô?Y>L'úLo?€ŒT?žô?ïäN¤ÔBâ?lܾ×éæ…?k±[+½o?lܾ×éæ…?ïu#!ÏÉ?ƒ¤uè×¢.?'[›ÆÝ©?ƒ¤uè×¢.4FGL J2040.2-7115¿ìøP@¤§ÓÀAs–Б}À9èFžÀ<<é•Zo¸@!Ž^I·?úIޚTª?¶UˆÞ
ŒÌ?¬_‡œcoÞ?÷ƒmjW@H­Ù©T?ï§hß½jY¿ÛÄþø*¿Ô;ýÊ
ü¿Ú&æô–?r¿Ô=¡ K¤ï¿Ñ*=áb.AGNbll3FGL J2040.2-7115PKS 2035-714?ïõŽ"cM6?M1>y¿ðO?Tâ×9e–"?M1>y¿ðK?ïø"e	a?cÊÛvñ`G?OvkƒÚv|?cÊÛvñ`H?ïÙL¡ÿ;?ttŠV$Û?sY¯bv‹?ttŠV$Ð?ïg*&Nä?}äž\ˆýù?"º»6#¬?}äž\ˆýý4FGL J2040.2-2506?äN¨sB£ÀA4'¾‹ÁÀ:³íضÀ<i"`šu@qàqo@àú)&j?ÈQe£Gî+?ÂOÒ:Ê×)?ñÝ t-Þ@7 ¼c?y¿æ*#õ¨Ž)¿å4¢žûÙ¿çe-BŠ¿¿ïÿËý™ô2?ïý1¹¶o"AGNfsrqPKS 2037-253?ïÖ+8~—?x«h'¡¸?têcý@´é?x«h'¡º?ï'Ì×[?rTxœ?‹zŒÊ)9?rTxœ?ï[ïÇCœU?ˆ'ïjÛl?"'Œu5?ˆ'ïjÛj?ï3JŽK?ŠúÊLyô?™œMö®6£?ŠúÊLyô4FGL J2040.5-1705¿ì Áèd¨À?—‰Åæÿ~À9ÇlÝxì{À<.œ×%@™ø÷øõ@l—E+ƒ<?±úëC/Ÿ¿›V)úœ¶&?åçÐ^QÅ@˜gu/,?ÝZr§½HË¿åǞ¢ŸÓ¿è¢ƒý†(¿ãδ˜ù`ª¿â~5ZTà,¿ïÿ»lR8²AGNbcuTXS 2037-172?ïþ:"âÇo?$äág¨Ú?,W±Ó‰4{?$äág§Ù?ïþ´Ól]?>ãD¡?$²Ïé:2?>ãDÚ?ïätu¨S.?iЭõ=Ä?k‹ŠW¬Ñm?iЭõ=¿?ïÿ
n뭆?
!V±Yq?²"ŠO5ƒ?
!V±Xé4FGL J2041.8-7319?î¨áeôú\À@ÜL˜_À:¯UQk,ŸÀ<•íÒt@ ò¾Íە'?û0íÕ·?È''·ÿá?»Q'ľ5…?ôÓæIîa?ù§zÓZÛn?ïÜCb¿æD¼'Âåÿäµ&Rz X¿É]F,4;q¿à•t;;?q¿Ù^¡IòAGNbll3FGL J2041.9-7318SUMSS J204201-731911?ïþõ%¿«e?#Á–o? ­¤I—æ?#Á–oM?ïÑî½pì?…Ó'+Yí?wž¡G‰˜?…Ó'+Yì?ïó6"îò?[Ô‰55Ð?Y"»æ"Ì?[Ô‰55Ã?ï"n
¾r?…÷ýIŽµv?Ÿ­'>¨1œ?…÷ýIŽµu4FGL J2041.9-3735?·X±÷mÀBž FÇd®À:qíâÇ
À<j+…¿È@ ÛB±Ux?ÿŠ7/+?»A*—®2¿~À!´(é?ÃG¥NX©@‰}G(ˆŠ¿íÖ±v/?áµü`äs¿ášmÔﱿÛSJÕù¿äh¸@"ÚË¿Àr€óZ€AGNbll3FGL J2041.7-3732NVSS J204150-373341?ïö`ì?JNЉÉÀO?S>'ïÏŔ?JNЉÉÀD?ïü¥~ݎx?Y†}^öc?:Ô	ŒG€?Y†}^öa?ïå3v.Ø»?r
Á«:?j̉Ñ'Fs?r
Á«0?ïí?öƒí?S°—ãÛ7?bÀ	|îÚ?S°—ãÛ7˜4FGL J2042.1+2427?Íå¡Æ>À%'Ó"wÀ9åÚ rfOÀ<$;¿É¯@ y2&ì±?þa8"œ×?´›m"<æ?'vx_ë¬?àØ¢mþ‹@JÝîZ¿èœf2d[?ïÿ8Yã¡%¿ã7; ¿þˆ¿Ô|_Ìï1|¿ågðßьO¿£a+'AGNbll3FGL J2042.1+2428MG2 J204208+2426?ïü"Wè0¡?:8Tïٓ˜?;Ý@¾zùý?:8Tïٓª?ïý@>F?TñoŒ"h?7mþÚ÷?TñoŒ"m?ïáœ2ú´Y?s–죭&þ?ncÍK¦U?s–죭'?ïÖýR,ü?he'Dð"¡?t9V遰?he'Dð"Ÿ4FGL J2042.6+1629¿ž<z¸ÛžÀ/*Îî<´À:Ä_½Õ¹À<]JÛÆdÔ@ ü›nÛÕÔ?ûC«Ë]a?Úù#¢œwš?ÈÜ!>6?÷€¬¹1@[K€1È¿ïøŽß#?ïÿt¿Å}M¿èJR]¿ª†ÁáÈm©¿êU8Á'‡?¹%ü"äÎÌAGNbcuNVSS J204242+162910?ïü…—ô?AæK¤ëqÀ?;ÓG€_dc?AæK¤ëqÉ?ïü<m7š»?cM&m‡?>–C*.Ÿ?cM&mŽ?ï'w6ªøÝ?"—܆5H)?›* äy?"—܆5H&?ïàÃk_íÚ?b [&¼!?o<" %£?b [&¼4FGL J2042.7-5415¿ÏŽ6ëktÀBä›A9†4À;G™Ò¤}"À=<ßP]¦@H;®@€"d®ÖB?Ñãz¥vÈ?ïÿûB«÷@FøðAF?÷'ïUÑ?í#Þ¬s;¿ˆÛ^¿‰¿Á–½FG.¿ëŒ#>Éik¿ïÿó€?ÖZ?î€Ý`í²AGNbcu3FGL J2042.3-5416WISEA J204241.98-540925.3?‡À\ab?È7ÐwL?ë^>èç¨?È7ÐwM?Î@Ý°ë?Ô$ø(â?èoȓÅ8¸?Ô$ø(â?Ľk97?±ÓgCgö?êÐ¥1¼;s?±ÓgCg÷?ÔÀÛw$?ƒó†BS|?ïy[ñù$G?ƒó†BS|4FGL J2042.7-0155?é›}¨À9iÂ;ySÀ:¶ãÊ?SÓÀ<_Öñý3@Ð3Xœú!@I:÷LÓ?ÇÐÜ&$?·vi¾µ‡â?ï:"£§@'èYp3Å?îò«ž~Û¨¿ê'ÇÅüÏ¿Ø̟ëÃ2¿ê3oce*&¿×'~!îè+¿èM?£ÙäAGNbcuPMN J2042-0148?ïî"nŒ?eŕœW?aíl'sã?eŕœW"?ïø¸a+,?fTþèA.?M{SO—?fTþèA'?ïy€%W|?Š¢•_?Ïþ{U–?Š¢•_‹?ïÀ¹eÝ?lƒÔmÖ"?£9M|'…?lƒÔmÖ'4FGL J2043.7+0000¿ëãkE=À8Â:îéWÀ:oÒ0¹Ü/À<\g=
¨@zî(½
'@n[þ-˜?¾¬ƒ×œ?›ñ"F7`®?àU'"W:@§6ycÄ ?î¹Ú¡÷Œ¿½Î6YX`ê¿é킺Z'¿Ý§]CýÜ¿Ú«zl­¨D¿ðAGNbll3FGL J2043.6+00012MASS J20434215+0001193?ïõi'ŠÃÖ?Sü	JÉä>?U-°êxRÕ?Sü	JÉäG?ïþƒ¨p('?Býâ?'Åxývî²?Býáõ?ïÁµ€Cï¥?€u&+KJæ?%?Þ-b?€u&+KJá?ïîÃ}8?OÜ£Çݤ?a<ø'èÆÛ?OÜ£ÇÝŸ4FGL J2044.0+1036?ïQeÓo'ÁÀ30%"ôÇÀ:Ìóf"‰À<UcV­Í@8[ƒˆ?曥BDH.?Û`ØóK¼—?ïÿۂr5¨@‰
]Qï@
ÊMó(O¿í.Ýãö_?íSq+¼Fm¿æY©ŸK4\?­(<	E£ù¿ïÿÏ=ÀTï?Җ'ýCDAGNbcu3FGL J2044.0+1035NVSS J204351+103406?ïõϏ×ìÔ?iBšùüé?T`àP&X?iBšùüæ?ïü'D^WG?ZÑ,¤:æ@?>ÅÝ
E¿á?ZÑ,¤:æA?îDá!ªœ? ÎN´EŽ?®+±íåVM? ÎN´EŒ?ï÷V è†^?U2£eïÂ*?QS¾.óE…?U2£eïÂ44FGL J2045.1-2346¿îa)¢ÍZøÀAm_Eà´áÀ:‰ =!É~À<|µwE²@•òôÿ›×?þéùc-ÌÂ?ÂÉë›ïà"?¶]΁¸1?õ`Ɋ"?ü˜k&ºó¿ïÚÍáŸÂ©?ïûû…Fü¿âµQñd[Ê¿Üè˜DÚÐq¿æX²é̷Կԙ}_QIIAGNbcuNVSS J204457-234643?ïû×ÈÚ?;!"´kJª?@ ßŸ"˜ƒ?;!"´kJ¿?ïØw¨›"?ŽGß»óDü?sÄ+²=þ•?ŽGß»óDü?ïâº1…Ú?q0n#šgþ?mEÎzó&ë?q0n#šgü?îʙš=Ã?'1/	Zµ?£Vn\#Ñ?'1/	Zµ'4FGL J2046.6-1012?ä…ÌþåMÀ>1Î_pÀ:ÀÛÉ¿ÒÀ<sÏÃøõ@ 33Yæ?þ†ÃÓÿÆõ?Å!#ü‰}î?³Žç á?ëjÑ?MGÜ?ý¸]ϓüw¿àDÝ¢x?ïøðâUË¿âó[Ao6¿ÜD""†ã¿Úþ;¤ñ¼p¿åa8^ì¢AGNbll3FGL J2046.7-1011PMN J2046-1010?ïûÈÈÑ>?@êsKǶ]?CÜÜÜ»¦?@êsKǶ/?ïò:Œ^·C?u*d'}(–?[ŠçB'wr?u*d'}(–?ïë¼àˆø¾?jÔLö1ïÿ?dCwB?jÔLö1ð?ï'OXNâØ?w9_jB´?‹¬)ìGJ
?w9_jB²4FGL J2046.8-4258?ïþ@VoZ!ÀCXœM©?À:Ö0Ï«¤^À<"üæp@>M(|ËÙ?þ>O%ØÝ?Ï]JˆåAc?њýôþ@:'FK@
ٝëØ¿î·3"Hø?ïý̞ÿŠ¿ß;!`Lò¿á9ýñ7¿ê]ß3á¿ØâÏØðÇ~AGNbll3FGL J2046.7-42592MASS J20464397-4257134?ïýIŒO?;¯/'jD?5³‡'MÈ?;¯/'j*?ïü0O£?Z"î™ê³??N}'ç°X?Z"î™ê®?îz"GEÍ?™ÂDaª ã?¨V»‹£/?™ÂDaª ã?ïç"\{x–?[íx"ÿN?hÝ£"‡jw?[íx"ÿN4FGL J2047.1-7400?éæǪ›>À@ì4~ŒÍÙÀ:ê»±òUóÀ<\{Xeò£@‰)Ô½\@Ü0ûJŽš?Íb@<??ªzK[Ú,˜?Ù0ù½EÆ3?ø¸+Ë	ÿ¿ïhšˆ¬âL?ã"×/Û¿ë΅¿G(3¿ÕµÔl©¿ïcȑԩ:¿í¾ÎaÍOAGNfsrqPKS 2041-741?ïåfß«ié?Œ½³Òá/?j™ T–?Œ½³Òá.?ïp©/q;%?§~'¿)Z?'êÚ؛O?§~'¿)[?î€PÇîÅE?šì<ñ£?§úó«À?šì<ñ£?îúj"?'EÉ<JBp? ^¾‰^—¿?'EÉ<JBp4FGL J2047.9-3122?ï`ýMuDzÀB±" ³Ô®À:bý%Z-À<køIRYi@jñõ%["?ÿô½±§?Äݑ€›pß?¿2&˜Æ
?úMn³<@&lXÁ?ïüšà–ƒ:¿è"@¡°¿Ü$.³q±ô¿Þ$)ªô4ñ¿áq¸¿y¨
¿æ^Ê@*'{AGNbcu3FGL J2047.9-3119NVSS J204806-312016?ïý€œáùb?ErŸU&C?3ûð4ùÀ?ErŸU&6?ïý|z—¾Ø?PÈp¿s¯?4+B	8ß?PÈp¿s®?ïïè"Sžu?lÿ¥7g?`l¬a‹ä?lÿ¥7g?ïàŠÓS¨l?X˜¹îøˆ?ou,¬W"u?X˜¹îø•4FGL J2048.6-6804?ïÒ2t>PþÀAì¹w…r›À:FNEÞ1À<w3Ï:eW@[9ë3?H@êùÞ}Ï?ºÃ¢Ÿ¨?¥4V@Jë-?ìŸóOîU@'Le¿ïü">`¸Ò?ïú³ääò¿èbªºSM…¿Êå9ñ=o¿åãflE£x¿ê.ՀzŽ¼AGNbll3FGL J2049.0-6801PKS 2043-682?ïûOTm3d?AÝ£î
ÄD?B®K2rþ?AÝ£î
ÄE?ïõYªw?ŠPgù·û?UMò«÷â?ŠPgù·ý?ïÔµXªïó?uÁhöý!?u¥SªˆF?uÁhöý?ï¿Õö•,?rkd#«Ë²?€
'yÚ´õ?rkd#«Ëµ4FGL J2049.0+1647?í­vs;ŒÀ0¦ˆŸsÀ:¦ÖŽín-À<C瀭9Š@,»h zÊ@¬Å@'H?ß;Äý ?—ñ`CÑTá?Øó÷ÿ*˜@	è	ê§?îÐvoÈå·?ï˜þý–ï¿ãÿ‹Á>Ï¿çWÌ'ãt¿ÖâénÄú¿ßq+{ÙÀ%AGNbcuNVSS J204902+164727?ïíÆ Ò¬?eî8¬»ªþ?b9ß-Sê?eî8¬»ª÷?ïúÃÓG	É?d‹rŸÌ'ƒ?Dð²ãØÜ?d‹rŸÌ'?ﳪ‰ƒ˜?Ê:B]ïN?ƒ]Ÿ™î?Ê:B]ïK?ïÍ¿ÿE
ô?i4¶C÷á?y ]yÌ?i4¶C÷á4FGL J2049.7-0036¿îטLíYÀ:`Æ÷ µîÀ;ŕ$¿ÒéÀ<³YÿOÖØ@#­ieIZè?ø–þ–µº?ɺˆç𔨿¥L9iƒ&f?Üi•ûg¿@ßÇÓ顚?çFyáîG¿ïÿþøþ"?ïÿÿ²}@?Ä/Mu~²8¿ïþø?ïñ"b"4AGNbll1RXS J204921.6-003930?ïþ‹‡e§
?'°ÔÞ(òv?'G‰¥Q?'°ÔÞ(òÖ?ïü©ýO¶0?Zé×3¥a?:°'Nr4?Zé×3¥g?ï ºòއ~?†)ûÀñ'À?‡ÑCH^ g?†)ûÀñ'¹?ïî­¾ŒR0?_¼àh"©?aRAs­Ï[?_¼àh"¦4FGL J2049.9+1002?ó?`À4µt'yèÀ9FÛeNÀ;×/(·Ä@ÙƐȐ@'£}H*;?±âò~Jf?¸)ÙBQ@
£ì¤©(@h©ÿ˜Q?ïøkK¨tÿ¿á­#ŸAyG¿æÚw_²íþ¿çL£FÁ…q¿ëC®á){$¿ïþh@0FÅAGNbll3FGL J2049.7+1002PKS 2047+098?ï÷uHf|?R¸¼"Ø+?Qo3ÑP?R¸¼"Ø+?ïï5NYb`?w¨iDÆhë?`ʱ¦ Ñ?w¨iDÆhå?ï
é
O]?"G"V©Æ	?ž¢ÍþV`?"G"V©Æ?ï˜Á'v)y?s¸Ës0¶?‰Ï¶"u¡–?s¸Ës0´4FGL J2049.9-2453¿ÕYþóÀB¶â—À:úÎû{6À<_ü@WÞä@´wWû>¥@nxžwNì?ÚÅ>c?â öàqšL?ïH'AÖ@xh"<]¿ïO>â=ø3?Ô_ÀÚÑh¿ÓñS)rÀ¿é{'¾Šêª¿ë{H`A^?ºdÈA!ÞLAGNbcuCRATES J205011.52-244811.6?ᅥp)Ó?ƒté`¬?€:^cõ‹L?ƒté`¬?ïüáw¹,?TyUM?8ôB7fœŠ?TyUM?ípûa*+Š?¡ŽJgwj?´x$ö®£º?¡ŽJgwi?ïÚ®æA[:?d«"¸^Im?r¨ŒßRcV?d«"¸^Ie4FGL J2050.0+0408?ۜ™ÏðàüÀ7ùb¿ù'À9r{'pÖ,À< ¢ûB+@\Ø%ñVD@BÌ}òt&?­I¦èÃ?qßKäâ?ÅóH6¥ƒˆ@P5Þß?Æ{Pða§¿ãOÅx¿å›Èé}±¿äb\¶º;Ñ¿Ü]/ñ_SM¿ëçZ¢bëÞAGNbll3FGL J2050.2+0409PKS 2047+039?ïç)>@°Ð?cdÓìŽ]\?hÖÁ¿O0%?cdÓìŽ]Z?ïýî^Tc?J£L8I<?0M
\å ?J£L8I3?ïÆ·ëÒ?€BțvÊû?~<ž¤
j?€BțvÊü?ïéÀ¤1¢+?VNÀ¸B*¬?f?[Î]Öf?VNÀ¸B*£4FGL J2050.4-2627?ïðn9Ç-tÀBbBAÃï®À:)ÞÊü5À<=BùyÔ@"»ªŒÖ@skd?¼‡¾ºÌ€?ÆÅÓ^a_A@
d²ú"¯u@‹j:±VÐ?ïîÀ!ß'¿Ð'9@=‡Ë¿ãKÈUnÇ^¿á."2Q‹ä¿è|J°j¿ïÿúâôAGNfsrqPMN J2050-2628?ïú&)?JGê÷ÃL?Gg³[´‰?JGê÷ÃX?ïýŒRò»?J+púø?4hj+K?J+pû?îUÒr$Ÿ\? H¨f&?ª¢Øݶ
4? H¨f%?ïúúÈE à?4:Pªâ¬ ?DÞé|"?4:Pªâ¬Å4FGL J2052.2-5533¿ëËb'0ÀCÇÞP'ÏÀ9M™æÆsÀ<-º9LQè@}»ÏN‡M@
hn~bÜ?§$H£v«ó?±ÒbŸÃý@$]È23Y@µ9"÷ƒ?ïÿ…]S˜¿ÛðŠ!«¢¿äÖ¹µ˜Ó¡¿äf;Óë¤ÿ¿æßyýò߆¿éà CAsAGNbcu3FGL J2051.8-5535PMN J2052-5533?ïÿ1qI?W™ó¨‹Í?™ÑÖàœ?W™ó¨‹l?ïü€±S÷I?XBÐëÜèä?;úu`Eµk?XBÐëÜèé?ï·ßÂÛÄ?€žÐô¨k?'I<Ï?€žÐô¨k?ïÿÈF‹Æ¬>óþQŹµ>ûܺª
>óþQź[4FGL J2052.5+0810?ÛÌX¿'@9À6H†zØä2À;Ӆü-ãhÀ<ÔÔoX}p@#­w§Ši?ì6q¬?æ\-Þ	¶?ïèø5u@Ä	_$RÆ@Êmˆn£ø¿¤	àmW`¿ïr}šàl¿ïj¼Â´Ž?ï÷V¾}©¤?ƁWƒt"¿Ñd§I……AGNbllRX J2052.7+0810?¦(¶—ã?€'ía;i?€õÒZò?€'ía;j?ïëeÍíé?­q+ð('?dš2ñ?­q+ð("?ï3Q-Ä_?'	ñï*Àã?™•Ý:Gsð?'	ñï*Àà?ïëŒãÄå^?iÍ|š†Þ?ds;¢ó?iÍ|š†Ù4FGL J2053.8+2922¿Ý°› ¿'À#´§qÉpøÀ9[¡ÔÑ~À;½Ca~ @ ïû_‡O?÷7קò!ñ?¹e1³rí?ËcËV€b@ÖKìgœÇ@	äQ»ßi²¿îâ/àm¿àÜ ý¦‰l?мj^ÄпÂåр´¿Ù1:_¢Qú¿Þ³+;-CAGNbll3FGL J2053.9+2922RX J2053.8+2923?í¢µFO¬?®xWï?²ëòU͂ ?®xWï?ïÜ"]?"iÏÄM|P?qõó¶Q€¦?"iÏÄM|P?껢'³Ëÿ?°f'ö©e?Åu¹0Ð?°f'ö©e?î͝†>á?f"u]s?£&'œîÔ?f"u]t4FGL J2054.0+7024?ʂtËÁ«!@0cجëÀ;½¾<RÀ<L™iÈñv@ 
<ÿdÐ@í-zŒŽ?ÅÀæå|Ç¿èhV"ú?ÊkÅJøL?󏐬5'ª?ïâp½Ø=C¿ì€"'‹á¿ÉÕ`ÅÂu¿é"²a'•i¿ßdIÁ1濧ÔŒ:
"AGNbcuNVSS J205350+702404?ï뛉©pÂ?jéàƒ'Š?ddvV>ö?jéàƒ'‹?îì–
Ü$Â?³ÅP§ZP?¡6ŸR=³Ü?³ÅP§ZP?ï‹z–ž¨¤?ˆ§•2™ª#?!ZXU×2?ˆ§•2™ª$?îuí¶‰?"¦dF@ýÊ?¨¡.t—gø?"¦dF@ýÊ4FGL J2054.5+4731?ëò¨§?T?úG-ÉÀ:|sÁ˜¼$À;àý÷Cõ@"
d|¬Mü?þÆ*\}?Ì1°|4.?¥&8à™?ØÏ1Ì*æ@¥4L?äæ†ý_¼©¿Äè'Ç¿ï³Ü:þÚ?äc=¬ˆà¿àւ""F¿äØ'sâAGNbcuNVSS J205432+473338?ïñÁºˆuh?_O|Æ3Ö?\|Šï3®?_O|Æ3Ó?ïõìzõI?za6Ép?UÈ'
n?za6Éo?ïh4Æã¸&?´7ÉEo¢?'ùg#ˆûn?´7ÉEo¢?ïë)unÍ?\˜)·þ³?d֊'ç2.?\˜)·þ±4FGL J2054.8+0015¿Ñü¿[YzÀ;äÚ	Ì2À:")¦ÂwÀ<O®‰ë¦­@!GáõRýÔ?ý!þ¨+¡?ÀY ãOp¿o+'\2¨@?²H`þàì@P¹Qð¸?嬗moo$¿ëåáℿÅf˜egÿ¿Þÿ²þ æ¿Ôâ5_wn¿Ú¢5_wnAGNbll3FGL J2055.0+0016RGB J2054+002?ïû·'†-š?6fÆÙ8?A#açI–â?6fÆÙ8;?ïþÀ<£À?<x¨É^¢?#ü5Ä(?<x¨É^Å?ïö×R"Ó?_œ\Oª¸?SØQZöX—?_œ\Oª¡?ïö¤ˆt?@¨ß| oÐ?R¶ïÅÏð?@¨ß| oÇ4FGL J2055.4-0020¿æX'ÂèÀÀ;sP]¥À:F0l¯UÄÀ<<¥5¯@ ê&dä?ûäÀ>Ië?ču‰nÿ?´wÀÁP»?ôô¿%D]@Lyµùw¿ïܕ'2Ê®?ïú«bùÌ¿êRÆ«ú?±1¦@F¿àûã:Í[h¿Ù·ÿÛ<§AGNbll3FGL J2055.2-00191RXS J205528.2-002123?ïüÜ#dø—?>¾ P´xþ?9äØ;En?>¾ P´xÕ?ïû€ž£?cqw—ä?AÿÐõ…t/?cqw—á?ﲠУ4K?†\AÏöF;?ƒWË×2í1?†\AÏöF9?ïâ?/EÞ?a›C{ ·?mÀкø!Û?a›C{ ·4FGL J2055.4-0504?çjõ×-U À=ÎðZpŽÞÀ:÷ÀªšëÀ<˜ëô°@•\­€k@ö¤¼ãJ¾?ÈWûØð?±*ð¬IJ?å¨D€b'?û/3÷Ô7z¿äûÎã''%¿Û•ýÈX¿çk(½Žkh¿ã'ßx ûŽ¿à?¾øMÚ¿å%:|CGAGNbllNVSS J205523-050618?ïõú"IÔ?Kô½"°ÌÓ?UÒ
÷lZ³?Kô½"°ÌÔ?ïäÕ.Ï$?'¢RՓ2??k*Ññ0ۜ?'¢RՓ2=?ïÈÃÓø3E?z'Ø´»ý?{žæ]æ?z'Ø´»ø?ï¾3/>
é?læ æ³?€s40}E—?læ æ³4FGL J2055.8+1545?î˜?ò!À2"f¥P‡À:‹Ÿ_¬8À<>À//˜t@E'Äë@¢e㉧´?ÌÕY8U†ð?˚KäÚá?ü=W(ÛÁ\@Rr{r'¿áëCII?Þîs恩¹¿çÆIƯc¿çv?!}ÿ	¿ïþadžæ
?ïô€ÜqAGNbcuTXS 2053+156?ïïS4??k(á<Pa?`í¬ËÀýø?k(á<PZ?ï݀¶¼-K?Bßò1.*?q?¤¡éZx?Bßò1.)?§»é? O$Sµc?¯—…u"As? O$Sµd?ï´ú@fn?vm
7"Wý?'Á\¯æd?vm
7"Wü4FGL J2056.2-4714?ç‡!ŽÀD1&|k‹iÀ7Š8|HOûÀ;"K}¬Ô	@k?jyž@ÒΤ=aŠ?"'p€Eµ—?»|ûÔ!Tä@"Ô¦°)(@Â*/ÔY¿Ä>ŸøÙE+¿â›SíNM¿çX'AƒÍ¿ça''zï
¿é‹¤ô^¿ë4ÑΔM)AGNfsrq3FGL J2056.2-4714PKS 2052-47?ïïå%U"?YL'DŽ?`Úªkè½?YL'DŽ¡?ï×j$z"?Š‹Çû=™S?tJým·"?Š‹Çû=™S?ï¡ø¥­£?‡§½<›?‡Öœ"—.?‡§½<œ?ïÞº¶Q0?f4'ÛÚù?p÷¢¤×gŠ?f4'ÛÚü4FGL J2056.4-4904¿·l¸ŸæÀD)GA1MÀ:Õ¶;ÏÆÀ<IjÃQ#@Q/@4xƒ@QÈ"n·?Ù1ŸY?î+hߝâ?ÿoœp
¯@ñËß¼é¿êå¡z8«B¿Åö
³¸(Ñ¿é­VN¿í3oce*&¿ï齞[ :¿îíÑ9*AGNbcu3FGL J2054.8-4908SUMSS J205613-490415?îÆîZÖ?¦JÚJÇ?£'Ê_'•?¦JÚJÇ?îò†?S1?±¢ÆÁAٌ? ×œ
Ìî.?±¢ÆÁAً?ì'ùÔnY?¤#ÿP¢E?»p1_¤5?¤#ÿP¢E?ë@@­';?²2]kË>Ò?ÂþÿýI»?²2]kË>Ò4FGL J2056.5-0202¿è™QgÞ;À<Ž¹¡vÝ­À9ç
›dtõÀ<:"ŒòÂ*@M@NN†@‰êdHR?»äC`ýÆÀ?À¼Ÿ9@>@ ¾×@Ä@I'zìZ\¿k
Ñ¥'¿ß*m¼Æð?¿çÒ·'¨ä¿è0¾yLòø¿çôÝøn;G¿ðAGNbcuPMN J2056-0205?ïûy•àN9?AâÀá´ò?B¨~Ǫ?AâÀá´ï?ïþ¿}?DÅäøØ?./'Ñ?DÅäøÝ?ﶄ~?~€KÑ@%?'^ú z™
?~€KÑ@%?ïôJ¿z
?D£Œ8)è?WjÃê[?D£Œ8)þ4FGL J2056.7-3209?î[68:ÖÛÀC¯!JÓcÀ:ŸZ·ÜzÀÀ<G{4SÄ£@ô¨^•@¤Ø&"»?ÅûœÙj?³Úx±íxi?äú›qàíì?ý¨å|qÀ¿àh)µ/ë¿çóÂâæ¿äŠ‰Ü¿ïÿÿÊPË?ïÿçÁŲ§?ÀÍ<HۑAGNbllPKS 2053-323?ïþ¿z:EB?'Ÿeÿ¥-?$\[«Î?'Ÿeÿ¥?ïûCRâÀa?k†n
4?Bò´tþ~O?k†n
4"?ïP«%+´? `ÿ>P´?•ê›Z‰|H? `ÿ>Pµ?ïýùGxË?3SL…}žc?07Ä9¡B?3SL…}ž'4FGL J2056.7+4939?ʹ7£…ý@	<"?¾À8c}}Ú À;i!Æ#e`@!p±E\Öp?ýMoõ[aP?¨³"?ãDÞ?¡=¢^6?ö­§%sW@	¦"Ö/?Þq&þòcà?ïð¦%™½¿Ëä¯A¡‹¿Û'$l ¿à]*"As¿Ô¾Ô;«ýŸAGNbcu3FGL J2056.7+4938RGB J2056+496?ï÷íôVõ?JoˆmĒ×?P$Rýn?JoˆmĒÝ?¾6?ªÒóK4?Ž™xrz ?ªÒóK4?ï#WÖT<?˜òH¥®6Ú?›œ•5xq?˜òH¥®6Ý?î´,𷇬?™Žàè«û?¤½0ô‡…`?™Žàè«û4FGL J2057.4-0723¿î¶¬e¿À?P]…TÖÀ:'%üéË
À<Eí@
@o"&¾Þ@pHðŽ?›™#'"?ÁÉÁÕwì ?ùLÝF—"@SãÉ®¿ÏºÆdþ²M¿åëðž¹2¿é(ôëÏÇS¿êîb›Ö‹¿ïë[rž¿îߋ€Ò"wAGNbcuPMN J2057-0719?ïüwôä\š?Bþt«­ª?<@XÝ6¼?Bþt«­²?ïì\ÀÚM?ˆ…ùlÔ·š?c£?%ÿ²=?ˆ…ùlÔ·™?ïÏÀG˜?z>DRè­B?xýòÜ4û?z>DRè­1?ï¸Ã"¯µ‹?q·¥™Ë?Ïԝ5?q·¥™Ë4FGL J2058.8-1442¿Ú
móMræÀA`Ľ3ҕÀ;#jęødÀ<˜dH~ôÓ@ ¬ˆ0½7@u×ÙôÓ?ÄrvŽ*¦¿«;Ž÷T4á?æ!EÊål?ÿ'g΀¿ÛÔñhˆ¿äpÝî]@M¿Û%⽤檿ۜ–ƒå}H¿â~äw
}—¿ÖH'¶þ.oAGNbcuTXS 2056-149?ïúZ­•Ü?>àŒd'?F•I¨À|?>àŒd'?ïû®ASÅ?`úÞ<(Úí?A½Fú°ê"?`úÞ<(Úë?ïôyÉDì¬?eú™'Õ¿?Wmv&¨D?eú™'Õ¿‰?ïàì»éñŸ?Yý~!(£?oD_·?Yý~!(¨4FGL J2100.0+2103?¥ÉÇû'p0À0#æÿëÀ:‹DÙMäÀ<(6'cDs@1Þ ôp@Ž ¤»5Ì?ί¹<:ï?ÀâÔánD?õø¶DË,@Íé/.è?íÿí@_Á‡¿ë>"E]¿Ù ²ýî­È¿ë€ y\¸¿Ý»lb&¿ðAGNbcuMG3 J210007+2058?ïý¬|³?=3¾¯ÓgP?2œC'i¨?=3¾¯Óg7?ïý䨁›?MÇjŽx??0Ú»÷[.²?MÇjŽx@?ïšÙç@®«?‡ÅG
u4?‰I†/ÔUs?‡ÅG
u4?ïïÿïèXì?M\8/‹Ž*?`§?M\8/‹Ž%4FGL J2101.3+0912?ÚZʨ÷©À7ƒï(Ag©À:ã´+W€À<v*¦€2@ 25\XF@ÍÝ|è‰?ÁI¡¿¨ä;ÃS?åž6Kìg?ý¿SrB舿èÊ(­ž3\¿éãîâvWJ¿Þܳàֆ¿Ûú\}‹Ñ¿á¤TÞ~¥ø¿æÆÂâh?"AGNbcuRX J2101.3+0913?ïû½$]"S?7²BCæ@E?An‰²³'?7²BCæ@N?ïúe¨Å‹?bĽ–ÌD¯?Fi‰\éÏK?bĽ–ÌD¯?ïñ &>è?h¶6rVÑÁ?]ῳ'.õ?h¶6rVѳ?ïՌFˆzû?c
3»Ÿš?u9ܻ'`?c
3»Ÿ"4FGL J2101.4-2935¿ïî¸òR§ÀCï–AöD•À:pÜÀ<4!'÷¾é@ìò²°@Ƙã'4p?ÂNÙ¬Ú?ÇRÇ%Ãß@.Lÿy@
朌h-¼?ëR¼ÐÖFÉ¿ç.÷™ÿðç¿êí3¿Ë¤¿ç¿jäz¿ïÿþˆ0»Š?ïÿ¥ÂqÕAGNfsrqPKS 2058-297?ïø[·	?XD:/øs˜?N'#ÏóÖ?XD:/øsž?ïñ"s–þ²?z™æ4F¯?]»ÒžM?z™æ4F®?ïÙ _âV?"5ß:r?Ÿ"ÛôµS?"5ß:qÿ?ïâÇñK»?a~ÈÔÕH¸?m8´Dä†?a~ÈÔÕHµ4FGL J2102.3+4702?ïþå}AØa?՝ò#žjºÀ8¸lD̹À;9•zP(6@Fx M'{@'ï[m ?´1[}æF?®ú	pìý?÷òZ
7'g@¼¾"ºêø¿Út_Cý?ïþdž;îÄ¿áõ
=€>)¿ãmŽä3ñŸ¿ã´ =¸g¿åálˆ€ÃAGNbcu2FGL J2103.4+4706MG4 J210218+4702?慎B.(;?‰‡áXÝe?…^/tuñI?‰‡áXÝe?êh¼Ҁ?Ñ|•N+ñS?Æ]ÀµÿÍ?Ñ|•N+ñT?íœã×¼€?©~a'ØJ?³áBKù?©~a'ØI?ì©DÙ£4à?©Â¹›ô?ºµÙ2æY?©Â¹›ô4FGL J2103.0+0342¿ìZñ"Ž¼tÀ:îÊFà!À:j;4¦À<=EŒÒ
ú@e`ïYÂ@¡¬Wâ?%?ƒo‹©?­Ï‡Ò?å—?¢,e@౫´#^¿ÜqÃL¿ä¢C çU¿æþ½c£>¿ãÛT"¼'ÿïnoês¦Á?é|ðKWgAGNbcuNVSS J210301+034411?ï÷KÏü"?PQÔ²Õ?Qh`÷þÿ?PQÔ²Ï?ïý2P¿VÈ?P"ÃrV»Ÿ?6mzI¿Ç?P"ÃrV»?ïÛR)Mx?ui¾«ÉÑg?rVòkYC¾?ui¾«ÉÑ^?ïö'On²?E,S϶‹€?S±a#Қd?E,S϶‹u4FGL J2103.2-2114?ÚrY¬ö`¶ÀC•_x5œÀ:ûXª¼ÍÀ<Ó׃	4@sS¶
"'@U>S!æ?È¿4ïb¤?£›¼£M¼:?Ûj•4°
õ?ý¢ë$PÂ:?ï?Äpݸ­¿æ\IÂkÊÔ¿â%!!¸·¿Ú¤±ÛYØd¿áœ?':z¿ïú"á%Ê?AGNbcuNVSS J210312-211216?ïúÍs£½ð?@¸"#í?DÊ1q?i?@¸"#è?ïïh^ïÆ?wÀÔ³ñ?`ø—¡:s?wÀÔ³ñ?ïá$.¨*:?r¢{ñd€S?nÛÑWÕÅÍ?r¢{ñd€Q?ïÅOñ‡ÃË?fLÍQRñã?}X<u?fLÍQRñè4FGL J2103.4-7816?ì™O¾»À@'óÜNôÀ;ºòù‡?ûÀ=Wg:¡¼~@M°À§¥v@,—½÷Fô?Øü>ª_º{?ïÿÁ¶ïö@—»=XP#?þΚ,f?ïغadw¿äz7i"ÙI?à)Ñ =ô¿çÍ˚¥˜¿ïÿßéà
¿ïÉöž'ašAGNbcuPKS 2059-78?젖ñ<k?½#jÅ]žj?ºûHv§õ?½#jÅ]žk?àÚÀªóà?×ù8'WØ?ÞKÒ~ª@?×ù8'WØ?åÇ-Ò®ã¨?¶ú»¬§³?Ôq¤Z¢8±?¶ú»¬§³?¸¦@¾"ˆ†?ª ËÿMÿÖ?ìë7è;®î?ª ËÿMÿ×4FGL J2103.7-1112?ï"µ®_?ÀA4Z¬1À9ßñQçSaÀ<hdÓ¿/U@ÍB§šcC?üŽ`¶#=?¼¸KTg?ÝóB¢'åÆ@ @9«ó8@r¤íà˜²¿ç7àìêO¿¡qëCŸ*í¿ËJl_Ϟc¿æs?ã­¿ë¯eŽ$Æ¿ïÿœ}y¨cAGNbcu3FGL J2103.7-11131RXS J210346.8-111335?‰n.OcÕZ?'ð—Ä¿ñ?ïšGFÂpª?'ð—Ä¿ñ?¨wˇð)d?¿—@¤ç{?îxƒG€ýj?¿—@¤ç{?¢i³ßrs7?—¿<?2ºU?îÙdÂØÍ?—¿<?2ºW?¶ÙÊÀdã?¦ô½õ[1ó?í$Ƨþ"c?¦ô½õ[1ó4FGL J2103.8-6233?îy–Ÿ"ZÔÀCyÅoÀ8ó¤>aeÀ;éµ³¬@wèºéö?ýº›
7 ?¦¢,+ܨ?»¢é#šŽâ@¯.Ìț@
{H!+ô¦¿Ù/F>¨²;?ðFyŒ¿ß¹õ¤ÝD"¿ßêoŸõÿ ¿åU¦$ÂW(¿àò''sã'AGNbll3FGL J2103.9-6233PMN J2103-6232?ïá"z»_?l²Eh*1ç?nÝþ…D¡?l²Eh*1é?ï	<PÓR?¶åC¨?žØuüE•¦?¶åC¨?ï!FàS‹?–uY1̈?œ;×#õŽÆ?–uY1̈?î¥Ú¢yŒ?'Ô—ZS<?¥¢^EØg'?'Ô—ZS<4FGL J2104.0-3546¿Y<$þŸ'ÀD´%®æ1ùÀ9Ì "ˆÞ`À<FŸ°4@™ãtÙñ£@ÁDÙMä?³·»B¶³Ü?¡5žPJ?êÈÇ.¥/@ùçb$b¿ÑB°Ž¨¥¿áÊa¸¼¿æċ_Å¿àú,hJl¿èÅ-0º²ï¿ïÿÓ?,» AGNbcu3FGL J2103.9-3546NVSS J210353-354620?ïþˆ$A?&1?`Æ?.—}¿Ëí?&1?`?ïþSÔsç—?E6wˆ?*¸Á†žf?E6wˆ?ïߌAj5~?qBãÜÚx?p9ßJå@à?qBãÜÚt?ïÿF´®®)?fžd?)j*:É?fž'Q4FGL J2104.3-0212¿îý[X†À>Q2ƒ
À:«§…§WÀ<` ä¶1@!ë_ð«y?ù1†U7	?ÃÉS¯-Õ?¶Îu'ãö?ó£Þ–ù¬@Ògd¾­?ïÒÀÓoS¿î,QA¼
¿›j˜ò|¿¹Ëx1¯·¿Õz«Â»üÆ¿Û쑎2]AGNbll3FGL J2104.2-0211NVSS J210421-021239?ïþ®É¨3†?]ZE‰1o?%e|dzL?]ZE‰1T?ïýàšÌ?G¡²zU—‡?0û)Ÿ‡¯?G¡²zU—~?ïõ½yžs?[šü­R©È?UƅÃý?[šü­R©â?ïêšÃAo?Teȝ]çœ?ee<¾û'¬?Teȝ]ç"4FGL J2104.7+0108?ìªäU®`À<ªà¹ÜÀ;®ìÀ<~̕ohn@Kîí3»?þ…ä*·c¯?ԉ݁%?Ìãݵ}Oâ?÷£›0r@µ
$F0f¿ï ŒÒá¹Ä?îsóãqT?Õ%çۛò¿àè`Ļܿç[gà$¿àQþÐUAGNbcuPKS B2102+009?ïþœðƒÖ?(¸ŽjO?.–0÷‰˜?(¸Žjc?ïýŽºÛ¬?VŽ_vase?3Š)"ŸVû?VŽ_vasV?︧§Q.­?€2ºÅv;?Ö+´T¡?€2ºÅv8?ïîRë"?QŒ¥Ý0å?aü­lýz?QŒ¥Ý0äû4FGL J2105.2-5143?â÷«Ÿ?'PÀD¹Â.äÀ;.á"ÚîÀ<‰"'Þº@yÝîÞ¦@E¦'¶(F?ŤK¹¼Ïª?më«¿säL?ª%vkí@ô¶ùPäI¿à|¿n?x¼¿èr@úœñ¿å­A—$¿ç™¯Ôn¾¿ÚQ¯<Ü)¿âÚÒê?¬AGNbcuPMN J2105-5145?ïýH!«4?0Â>nÎ=?5¾ó'¦T?0Â>nÎ@?ïþ»±…yÙ?A!Âb7d'?$Dç¨bok?A!Âb7d|?ïãÇs§Š?m'ñ|¼ÄY?l8ãŒXuó?m'ñ|¼ÄV?ïý¢̉ì?$¾^ì²æ?2ïћ°¤ä?$¾^ì²é4FGL J2107.6-4148¿µZ Ù‰ÂEÀE>$_ZÙjÀ:'
[2U¾À<|2;¼n±@N ?ûîx@Êi`êM?Å–)̓×?»¸€ºz¾?ópnAüú'?þ0«#uü¿ÏkõÇl房à/ž˜\¿äo¾Sã,¿å`ºÀZ΃¿ê²M?Mó©¿ïÿ&ñÜPÎAGNbcuPMN J2107-4145?ïÃüÚ¡?w²÷(	¨?~'¯öF?w²÷(	¨?ïÊþôbt?‡³g°Ðƒ1?z€ò…ÎÅô?‡³g°Ðƒ2?ï(Žì¯?'ž€¹)?šî"j*?'ž€¹) ?<q?…Ëdbì«í?Ÿlxqß-?…Ëdbì«í4FGL J2107.9+6006¿ä(YÛr]@ ØÀßXÀ‹À9î²-å™À;'KZqež@"eæ
æ@ß8úóPÅ?Ë$kYÀ:Ã?ÒS:»@gæ³þŸ®?ú˜€â¾{¦?çôS>kuš¿ÑDŒÂÂ#¿é´÷!¿æ_iQÓ1k¿ï÷äÞ;Š¿ìue<š»AGNbcu4C +59.33?Õ3"–°…?̉Wڍì?åsf5´§¼?̉Wڍì?ÍPVˆAÆ?Ï#Ÿ)Û#?è«êï?Ï#Ÿ)Û#?×r;\we?¶"«>õª?äFâQÄ}Î?¶"«>õª?·
¡ºðs?šqù&ÃÐÕ?í~KÈ¡ò?šqù&ÃÐÕ4FGL J2108.0+3655?êጎtÀÍ
Œ°}À:ÊÓÎHÎÀ<&¿»lR9@ x¿úeñ?üe&*64o?Á?öût€?ÃΕ¤Âl¢@ª‹ÄÄÀ@̝–~\&?éåïé1‡b¿æóóiâr¿Úª|€Y+À¿Û
ü]^*¿×Ù#"™Þ¿ëS9bøÝAGNbll3FGL J2108.0+3654TXS 2106+367?ï©ù-
†?€S"².Þ?…¸ô½^O?€S"².ß?ïæé9è%`?"'Hpj8¹?iÆÚ ï?"'Hpj8¹?îõáp/v?˜$'	:†? ¡èÿý?˜$'	:†?ï7 x?…ŽP¤6»?ÿýYñ?…ŽP¤6»4FGL J2108.2-2454¿ïdÊˆ€ ÀD¼j~ùÛÀ9î/²u2²À<Sîe£ÈÈ@³P–‰@_êÄ.˜š?¸œ£å"5?§¯ýˆ¬a?ê¨Ñz±w@q¢Æi}¿Ù#ñÁùµ
¿ãô~ø-£§¿å¯Z@hOö¿ép'D¿é0aœ¨¿ïÿì^ãe@AGNbcuAT20G J210812-245233?ïþÛ7¼wà?Å2¶ÐW
?"L"8ø?Å2¶ÐWÊ?ïþYî™&?EïÓ2¡.v?*anÆ?EïÓ2¡."?ïÞ¦X#õ?pQÇÅRÆy?p¬Óî?=?pQÇÅRÆk?ïúÁˆ´xF?8þ™øšàö?DùÝ.å]?8þ™øšàý4FGL J2108.3-4824?ánÉBŒíÀE)Ëeè'À:ÈV%¦'¶À<P–ÔÃ;T@æÅÎ*ñ@B÷<@?ÉÔMI´ÔÞ?'4ëïý©?ÃÏÖ¢"@QRÔäv¿®pXœhß¿åF/ßÁœ¿è58@¹-´¿êÎô$)ªô¿æ§­ŽC$B¿ï]6=©¯AGNbcu3FGL J2107.7-4822PMN J2107-4827?ïü‰˜ä?>Ja$¿™%?;·Wc8ÚÀ?>Ja$¿™]?ïìV¡æ?|:#"%¸?có©^å?|:#"%¸?ï¡‹™e?†‹£»Æðx?‡¾<Ù¦c?†‹£»Æðq?ïïJ1"g"?Mù•b3t?`µÎk˜m?Mù•b34FGL J2108.5+1434?è¶áèMЀÀ5¾p'IÀ9¿%ª´tÀ<#M"M@tN?þó'@"9¦û`?»ÿüOq ?Æ #÷V
@@ç6žË@žâ¾ü?°‰c–}Zt¿ç‡ª^7éɵ ÝD¿èûDå^³¿ïþgä맃¿ïna'·'AGNfsrqOX 110?ïúíð:?HmV†ß‹|?G€H?½H?HmV†ß‹?ïøV@¯Jñ?fFHõʀ®?N¦ýBÔ;þ?fFHõʀ¯?ï+š1?'¥x1D'?š¹à ?'¥x1D%?ïÌFté`˜?g{5u²A?yÜŋO´b?g{5u²A4FGL J2108.7-0250¿îì@QýÖxÀ?–E"}À:Id?D¹mÀ<cÿå(
e@<*žµ@z͹[ÖÀ?·˜SH|p"¿•4beÙVQ?ÞùI,™»þ@ƒàṗ?îñ/'¤ŠŽ¿ß'r¡L%¿á´M¯¶;'¿á§UCÿ3Q¿ã61µ"±«¿Û×[µ2AGNbll3FGL J2108.6-0250TXS 2106-030?ïìÝ©åÖ?[ÒEteå?c"Vâ*ß?[ÒEteå
?ïúv"Ë?jû$!­P?E˪%ìÖ	?jû$!­P?ïܙ¾ôø™?w.ü`ñl?q³ …ƒ³È?w.ü`ñl?ïÃ
–¿–·?g`¼$ð­?~z´ 4¤œ?g`¼$ð³4FGL J2108.9-6638?æUÙX– æÀCÄÑ¢À9‹á¸À<YŒ~þä@‡Ëz½5€@ãÔk&¿‡?«£cUdá?yž	>7á'?Ωu¯¯†@38üö¶*?éÅëÒK'Ï¿áS
æû¿äÚ?çvœ?¿Ü!¾@ÂèÈ¿âÂâ2ŸE¿äÎ%\°ÚÿAGNbll3FGL J2109.1-6638PKS 2104-668?ïãWB®Qˆ?`¼Òµ'"?l¨½Q®wø?`¼Òµ'Œ?ïô6×o•b?y_×ù8' ?W'Q Õ<ç?y_×ù8' ?ïºÁø&I®?<ÙzV‡?Oöm"œ?<ÙzVƒ?ï¿|¾Ü[?mrŽð¬?€ ЈéH?mrŽð¬4FGL J2109.6+0440¿À:¡^xW"À;䃧 À:f̧ãß8À<-Q{×@ЕYC@ÖÎãþAº?³ˆX(¶?žÚ܍"?ßÌ¿`Ón?ÿ`™56Ä?îÂL ˜?àöÚhµÌ¿æR,¾}¿à+›>µGu¿à¢–˜]Yw¿ïüàÎï½AGNbll3FGL J2110.0+0442GALEXASC J210940.09+044000.8?ïÉyä7S$?uÜݲ<Ñ?{C
äVmÛ?uÜݲ<Ï?ïéFàf?z0:½¾ý|?fø¹™ç"?z0:½¾ýz?ïŒ
êݞE?ˆ;(¼x¥?ŒýEH˜o?ˆ;(¼x©?ï%ã녔7?ƒˆ	s½;?›C'My?ƒˆ	s½;4FGL J2109.8-8618?»i¡õ¸×ûÀ=.î¢
À:ˆ^iAâùÀ<pär@!™lä.é"?ûdÏÝùDû?À÷g€æ¡?¥þ®Ç(H?æÿ'ö֌?ýltóG
?ílŸWŸ¿á}Ó %¤Õ¿á•,b³®¿Øp¤ý[¿È	û÷ݝ¿ß IaûcAGNbcu3FGL J2108.6-86192MASS J21101113-8618473?ïû¥¥>5?74`Ne€?AkÅk-½?74`Neº?ïüeUöX?PÜÏؐúÇ?<ÕPM?HŠ?PÜÏؐúÙ?ïòµ}ƒí?bòk—H?Z•Êø#á?bòk—Q?ﳺŒ"ËA?q.³Qôz?ƒ\ÞÍ/µ?q.³Qô}4FGL J2110.2-1021c¿Ø¶¨Sž#ÀA½¾ôœõoÀ:¢v0íÀ<@õ0™%@t››&Œ‡@°HàC¢?Ëç"Ï/~?Å.¾¯R¾?ð…£dôv@ZKë»ÐP?ë™H`–Üx¦ojñæ¿æÌ<6çô¿ìŸÂÞ6œ¿ïôÁ]'çü?ïÐù^#øAGNfsrq3FGL J2110.3-1013PKS 2107-105$?ï¶a");?…[Zrq, ?'gžõ±?…[Zrq,ž?ïÇÅ,—…?õšàóÎù?|i´=??õšàóÎú?îAÂÇ;YÄ?›'#ÀÜ?«ãӌJcÒ?›'#ÀÝ?ï™D: —?{BòA+jO?‰®þñwÚn?{BòA+jN4FGL J2110.3+0808¿ "$н'qÀ9ëOÆðéÀ9ÌŤº_À<6ڇ s@Ò¡ÍðŽH@ÓÒåëÄ?¸r¹ÛÙZ$?²)°þe @?÷™DrØ@{Çb¦ÿ?ï1ž2°¿ä‹a'¦ãÚ¿å$†È½¯¿ânå€ÍÅÆ¿íKòa±ËÀ¿ÔOG› AGNfsrq3FGL J2110.0+0812PMN J2110+0810?ïûõHT€?4õ!•m¹´?@+òÞ­ÿ6?4õ!•m¹ã?ïþ™´Éá?DïÓç×ø;?&d³gá÷o?DïÓç×øG?ïÊ<¢7?{ó&".¥?zá®ðqå?{ó&".§?ïüôêÓ;?'듙^ü?8_x©f&$?'듙^è4FGL J2110.3+0404¿á=$DmGÀ<@vžÂÎFÀ:œiW²n}À<T§i¦@  捓&
@>:}ªOÊ?È÷·1/"?¦FŒ~Õô?á6:Ÿ8?@©m˵u˜?ïî5!õÉ¿éV­@•ql¿à֋\¿ôw¿â:s™TÐ<¿×àcØl"¿é*''¥AGNbcu1FGL J2110.6+0403NVSS J211019+040418?ïýÊwöX?,%_Ycm?1¯Ä@M?j?,%_Ycn?ïþÖXlgR?>¾*>æ?q?"šy9ŠÑ:?>¾*>æ?b?ïóÕþG¶¹?eÄÀsD›¦?XTp'X?eÄÀsD›¥?ïõQ|é?DÂù6e?Uùé]/F?DÂù6u4FGL J2112.7+0819¿á{ƒ;ñbÕÀ:O9_JÀ9ìT3]û^À<%aþÈÈ@ 'òK—
?ü˜˜è™²?ÀüššËrÛ?Áƒœ—¥Î†@X¡ß¹8›@
,íZ`ô?±'l©¡y¿Ë¿ˆ®å±¿æi\ÜJ¿É ¹¿ú¿Ýù"ÏbÔ¿èîö«¢AGNbll3FGL J2112.7+08191RXS J211242.5+081831?ïúäxýT??}ô©ÃB?Dn"
¯Ü??}ô©ÃC?ïüõˆA?P•~|÷*?8S¿G
ó}?P•~|÷,?ïÔé"{-?xúÙ&
p?uö6Bit?xúÙ&
k?ïæ+ì{å?UñÎèªõ'?iûÔ"ß?UñÎèªõ™4FGL J2114.7+3130¿ëKˆ™8b0À'ÄÂÖ©ÅaÀ9ïÉ¿Ò‡À<œšÕÚ@›`Ú5k@(Ç\Jƒ²?¾Œó$?¹&äàÎU?ú:bÒ]0@6~jê¿¿è÷›bFœ¿Ú¢^¤¦#¿äŽ	Bžá¿ßë‹Ô´ø›¿í.Œ¥•P_¿×®à}®¬AGNbcu3FGL J2114.7+3130B2 2112+31?ïWiw}?œéP3?•ÒߑQ?œéP3?ïí`#ÞÀã?|QžQpµ'?bŸÜ!?Œ?|QžQpµ?îL¥Ûã9?·9=Ãr?«?¢AÌx?·9=Ãs?ïgôŸ)€?€"œ'â+7?"lÏýß?€"œ'â+64FGL J2114.8+2831?î!£õÂË&À+ϑ`4PÀ:-qRR³À;ØÔà—…@H'1·]@[˜fÙS?ÅóyÄ<0?¿Xòà\̊?öl¡«¶Ó@€?ƒ"´¶¿á·ü€Ä‹‹¿èú~¶¿D¿è•«}Ç«ü¿åtÞÏ-пïþÑÌæÎ?îU—¬Y¾AGNfsrqB2 2112+28B?ïý‡Â£Î?AŽ¡¶ç?3ÁïZᑬ?AŽ¡¶Ï?ïûkßé~¾?cóÅÿ0ë?BP€ZX?cóÅÿ0ë'?ïqB†æ˜[?Œjlã®yî?'ׯ#,ô¤?Œjlã®yè?ï÷,;GØÀ?FV|b۟?Q§‰pN€˜?FV|b۟q4FGL J2114.8+2026?îɧë0à°À39"úÖËSÀ;
º(…ZGÀ<zÙ@x–@ wÅ3{X@qæ¤å'7?ÍĊÉr$`?§ë#$iî?Ýð¥dSÉ@	EíãðQ?ïÿàŠï²«¿éC_›q
.¿áÅÛAÖ¿áí6ß»¿ØV}JK¿ðAGNagnTXS 2112+202?ïÿíÁLý>áçWgœWW>â>ù³¨>áçWgœV\?ïþ—™Òµé?Mñ0MO?&†bÔ¡]o?Mñ0MD?ïòîqàü?axÃ÷¯3?Z#ý>Å?axÃ÷¯@?ïý!fãÈ?'>jër?6ôÈá¿5ã?'>jëy4FGL J2115.2+1218?ïhQúªÀŒÀ8k•¢"À:B—Ò<èÀ<S‰®j7@ "¸ÌdÈ@B¡e?õ¹?·DʊRS࿘=~e¶"%?â5e<š»@w°˜¹ŸÉ¿Û9"5‰û¿ÙÏ~"DÎf¿æü€xá=¿ÏÔ<ãÚÛ¿èmH7§6:?ÏéÊÉàAGNbll3FGL J2115.2+1215NVSS J211522+121802?ïþ+Äæ8ê?1(ܾƒ…o?-C±œqb?1(ܾƒ…^?ïþ¨ÝpA?D''(÷õT?%r(ûïùh?D''(÷õ@?ïéH¹‹C
?tޔôqë\?f·Ft¼õ?tޔôqë`?ïúáL¡Hm?9ºµ©ö•n?DzÍzÞJÔ?9ºµ©ö•¡4FGL J2115.4+2932?Öö"1oÀ*¤$=Ìê)À89'T؟iÀ;u™ô2ld@î;'Ó+â@òŸYÌúð? ¼nþøå?»¤Ùh¼ü@Øú†C@Ѫc@l,?ïúû^Z©D¿ÞR%fÁÕù¿å7àAׁ¿ãùê<I\j¿éJߢ<€d¿î´ ~$É
AGNfsrq3FGL J2115.4+2933B2 2113+29?ïðE(¡?ZVV}}——?_u÷®½Ü[?ZVV}}—‹?ïð{DÏ6"?w. ÈEä?_	va'×Ì?w. ÈEæ?ïnt³ÂÔî?EH~îz?'1i‡¥b0?EH~îv?ïò>["‡Ó?L"óÌÎ*³?[ƒHöðYù?L"óÌÎ*"4FGL J2115.6-4938¿î¯N0(ÀE®6Á]-À:­Y-˜¿À<œ™µHKÉ@.­f*+x?ÿPpûëžI?Æ<,9
ä?¶X|ÀÞ?ñZë­ó?÷<T "ž¿ß¶,A§j=¿çûš«'"¿Üˆ%=|7^¿Ý:ŽÜ§5d¿â\LœÄß¿è òž˜†õAGNbcuMRSS 235-024179?ïüÞ¿ÿþ‰?3`ؾœ"?9
·â?3`ؾœ´?ïÙó€úb?†wö€Øo¹?su†?'Îf?†wö€Øo¸?ïè^'Nój?oLnÅrb'?g¡Ø±–!?oLnÅrby?ïD؈ü¹"?ƒ®ã»!?—dîàhÏs?ƒ®ã»!4FGL J2115.8+6753¿ÞæY •)I@*	"ãÿïÀ;Dœ)¥ìÀ<"!É~c³@!m£4"‰?õÒ¼›&b?×u»Cš?ãӕsš+@ryJ@;íÞrÔ?àcƒ'«ìX¿ïÒ5A€R÷?áóRÝóe¾?ïÅèít¿ç&~"j]l¿Ýqü¼Ô‡+AGNbcuNVSS J211618+675324?ïŠz³ k?†5eù_˜k?aS:7åK?†5eù_˜j?ïÕd¶"¢?•*Cþf×R?uxM¤µ¯?•*Cþf×R?îælÄu~ï?˜ÿa^|ï?¡™3¸¨?˜ÿa^|ï?ïH|²·|?'Ȉ.(?–ði©í?'Ȉ.)4FGL J2115.9-0113?ï¦Ç¢Z6À@'¼ÓZ…ˆÀ:M´ÒÛÇÀ<d•^¡v@Ng¹L½H?ÿùäwä=,?‡o vØy?ÀOâ€é'?û°ÔéÑÀR@šsPڎ¿ç*SÆP±É¿Ý‰å£©¿àâçÁDÙN¿ÜxwÀ«×4¿ïŒ~"ƒÕã?é³>¡%AGNbllNVSS J211603-010828?ïáÌ.'ø/?pôÉñ:<Ì?n3ÑmÑj?pôÉñ:<È?ï÷¿}'?dРʻɝ?PáÍÞ?dРʻɢ?îÙáb›Æ@?˜Ñ_7 Ñ¨?¢aéÖCœ?˜Ñ_7 Ñ¨?ïÊYÑן?pÌÎPŸ¨÷?zÓ0t+?pÌÎPŸ¨ú4FGL J2116.2+3339¿Ò~5Œ‹À%MOçžàÀ82LOcëbÀ;[í¤³©@¡Üí+g?ûòˆ-`‹[?¡Sʂo±i?¹.nRn÷@]Û	íÀ@¸Ü&$?æÇ·ÿá!C¿Ò½·†ªØ¿Ù"¾h…û¿ÙšÛ
,c¿âQßƤ•¿à`䡪µ AGNbll3FGL J2116.1+3339B2 2114+33?ïû=í*›Ç?@tÈç¸ë?CKUèP?@tÈç¸ò?ïîY'?tCGê<¥l?a¦m÷ïçU?tCGê<¥j?ï´ä…
?ˆNç_Ýöq?'ÆÜž½9?ˆNç_Ýöt?ï¸å¾õ{?kE<´e?Æ¸B¡,?kE<´k4FGL J2116.3+1015¿ÏÌIõ("JÀ9Ý˼+"ÙÀ:û,¨Õv¿À<e¯¶;Ð@ÇXÛch…?ðx
Oš?Ü¥0úØ#?ïÿì´É È@®-±éò@ƽñÿÁ·ù«
	¿ê
aw¤Q¿Õ©úºÆ»¿ëtÙé¿ïôL¾´ ?àV"Zî¹AGNbcu4C +10.65?ï›K×<P?ÉfI3=?‰-=Ê0ì*?ÉfI3=?ïšWóQ†?®ÖpHø8?‰j;Ã+ž÷?®ÖpHø7?ë÷0Í:¤?ª
IVO/?Â#<Ëk?ª
IVO/?ïÁ¥zÁ?˜1Dž‡?žËP®GÈ?˜1Dž‡4FGL J2117.4+6159c?ïóWQ©p-@!µo—g2À:²aç|À;ÔUÓq+¼@)Ñ,­Ýô@Ò¦-?Õɞoc?èÀ‰þ#r@
fr$àŠ@¼]Sm:k?ïþnÀ}>¿ÚkJw—¿ç<"Åý¦¿î-ë•å¯ó¿Ô}¢'¡Zƒ¿ï¡kTâ°dAGNbcuNVSS J211613+615920 ?ê'Ïûb{Ñ?Ɖl˘´??Ç`ÀvÁ?Ɖl˘´@?ØÄ™+¯‹?ÒÅàÜè¼?ãø³j(;?ÒÅàÜè¼?Ü'æzÕ?¸ÃƵ¼šÏ?áñ|>ŒÂ•?¸ÃƵ¼šÎ?ҜŸù~Ò??ÀnX·až?æ±°@–à?ÀnX·až4FGL J2117.8-1521¿îE;¯U¦ÀCp'IüÀ;Çwù5áÀ<hP?³t6@ÌYjÕa@ÏãzŽ;˜?Ñøòû4¿$?¥OiÒ~?̧Àä6Jë?û`¤$âãe¿Öa·˜ˆ¿Ýþ‰Î´¿à¶+ —ºœ¿çRÜ{–yT¿ïüt$•
¿?ï¶ý!ÿ.IAGNbcuTXS 2115-155?ïø'B!EÎ?R𮓔ù:?M¶÷zèÃ?R𮓔ù5?ïÔ‰³zE?…±¡Ë?uò;&Bܕ?…±¡Ë?ïNú"À?"ûH¼òªA?Ÿ> ­gß?"ûH¼òª>?ïÅ®—Mڄ?måk¯­ÓÙ?}(´Y¾7?måk¯­ÓÛ4FGL J2117.8-3243?ïÂHGˆ0|ÀEïÚQÎÀ:z[ôœïÀ<M\ú¬Ùè@ ZÛ¯"«ï@eÏ?mÔ?½h"£¾5°¿šÀ>ÁS>c?ßX´Ae¥÷@ËÃw?ë€FvÜÖ/¿àÀÁü28¿äVóAUµ¿¿ät9Ûr­¿Íy¨7—¿ãý먰AGNbll3FGL J2118.0-3241NVSS J211754-324326?ïóýöpO?T¬Žnõê?X÷`¢?T¬Žnõõ?ïú³cÃò?Z3zܦªÙ?E2pð7 '?Z3zܦª×?ïá-zËÚÐ?r§î:³=G?n҅4%/b?r§î:³=B?ïڦئÔé?bV!3O÷?r¬"¬•‹L?bV!3Oû4FGL J2118.0+0019¿Ä\ñ–ÀÈ5À?è">À:¥6nQsÀ<Wæ¯Ìâ@ø5˜hA2@ø'œ&;Ô?ÝíM
tÎ?ÚDôPÊ?ü@ÇÀôQv@SÐ|"`¿ßc[+J1¿ã­g¬·"¿æ*MçŸð¿ívjàžÏ¿è¦ÞHJG¿Àzz(ÓAGNfsrq3FGL J2118.4+0013PMN J2118+0013?ïñ­à>2?hÀˆùXµ?]̤?ƒÑ?hÀˆùX²?ïþ¹X¹Û?GA§·B9?.jtbH?GA§·BB?îª5¿my_?˜	øŸüÉk?¥\¤	(j?˜	øŸüÉk?ï÷=šÜ
?EÅ
—Ç9?Q"ËÜGãÌ?EÅ
—Ç74FGL J2118.2+5752¿ïŸNAæÀ@¹p]`-gÀ9Á;ϹçÀ;™j×o@àçñìA@	'C‰ÂŒ?Â>ˆ;xQ ?Ä}þ&×Z@TŸCý…Ò@˜öChµv?ï"]9–û¿çÖ´âË;Ó¿çtŸºšñ¿ç8×L''¿è©ç$f疿ï¾àÅýüAGNbcu3FGL J2118.3+575187GB 2116+5739?שּׁ%¢qC?…T²nõÚ?"Ôö—c®ø?…T²nõÚ?ïð9:?kGß6V_?_ÄŊáÃ?kGß6V^?î;+ W®?ØzeÁW€?¬MGåú…?ØzeÁW?ï³Íf^­æ?p>&æErü?ƒ¦hT†¶?p>&æErû4FGL J2118.8-0723c?ï¾D¤›EÀBhß½jYÀ:ª(҇ ñÀ<,=]…@öE(þüË@8\gßã?ÍuÙ`ƒùI?Áޅ†è!?택Âô@¢ašú—¶¿æpoiDg8¿ån8¿,Ñ¿èëõÈ|Ü¿í†Ëá•[Ç¿îèïwòå¿ïÿüoQÇsAGNnlsy1TXS 2116-077 ?ïÿfäƒ
"?ŸƒùFà?#ož»âi?ŸƒùFw?ïÖм#ñ?'+8ÈÈ}à?t—ó!îH?'+8ÈÈ}à?ïÂüâU?}SȖøLI?~úyŽÕ'?}SȖøLC?ïå­µ[ëf?Yó)¨ Òc?jRJ¤›?Yó)¨ Òv4FGL J2119.0-3317?äç qfàÀFbMÒñªÀ;Ykã}é:À=!Iâ¢!@ÉH±Æj@ÃRë__?Õ.³R)˜?ïÔËi~K@ëÿÛk@ŸÖ
=UK¿î~ߧz®¿ØÌü½«FÀ?Û¤]Aúv¿æ¤Dî¿î1Ū™œ¿ïöF"¤ÐAGNbcu3FGL J2119.2-3313PMN J2118-3316?Ø)~™y?Ëà°ÿø
?ãëyÀ³rÃ?Ëà°ÿø
?ãÆßޏ­›?Õ¿ÐÄvx?Ør@Bà¤É?Õ¿ÐÄvx?ÛONm{¸Y?Á`ÕâÔçø?âXXÉB#Ô?Á`ÕâÔçø?ÚcÇ.Òéí?ÀnŠ,-v?âÎh–‹
?ÀnŠ,-v4FGL J2119.4+4652c¿Ò lÈðÑo¿þ©Ü¨#$À;4ÒÆÒíÀ<¹?QN§@!~';ýP?ýBL
šµ?ÙzGĺ¯"?î£bۗjë@	÷ÿ=ba?óá–óÌëÖ¿ïøgàŽö}¿êæe$G?îÃ߈'3š?ÕW³%óà¿àb¥ç…µ·¿ïÿÿÊPËAGNbcuNVSS J211922+465026 ?3Â1?"¡ëS"'Q?ŠP3;OsÛ?"¡ëS"'Q?ߒmj&Æ?ؘ»§p"?à6ÉJìõ?ؘ»§p"?íHâˆ?¥oír…Ö€?µ¿#€ë"Ç?¥oír…Ö?Î2üT?ÁêðVœâ?èy³@Ü»¬?ÁêðVœâ4FGL J2119.6-1105¿ç¢·×p‹ÀBñŒ~($À:oÍuhÀ<KÛ$~dŠ@9"v¢s³@þZäR%?»§!	K>?³Ó}kÃl?õN¨‰÷e'@édZ&?ïìpk¢æI¿çóZ4ÿ¼
¿á¶ôžM›¿ä~q f¿ç™ÌYàF&¿ïïÀý¶¤—AGNfsrqPKS 2116-11?ïþ hQ¢Ç?,ú—"5X1?-ùzåӊ¹?,ú—"5X\?ïþ:Œã?H™D?/ŽW1Þv?H™;?ïÏè8fèÔ?|&òu¸X?xã̋•Ä?|&òu¸T?ïÿÑÆ'˜?
±˜£Ôü?‹Žvé`?
±˜£Ö4FGL J2120.6-1254?í'*#RÀCnş±áÀ:hß۝J(À<d×ؙŠ@ÁÊÍC?E@}!xö‹ã?ÀÍßÇPa?®Â_œ®Þ?ìܙÿ&ó@€×€ÚÜ¿åîO¾Úé¿ÑŽ)ùΎ¿çñÝþMx¿áõ!HÏþ¿êŸåãõ~¿ÓUžã/»AGNbcu3FGL J2120.4-1256NVSS J212035-125443?ï÷ÃK£íû?Jì›5ÝÇg?Pyh¸$
}?Jì›5ÝÇb?ïþU.,^õ?G3>$3ݦ?*­:·H?G3>$3ݜ?ï·ÊY¤?ƒ	f÷J?'
i˜¸VÜ?ƒ	f÷I?ïüÀMÆ:?.»ü´M¿F?;'ý'Î(+?.»ü´M¾ã4FGL J2120.6-6114?ëÄ»m í¸ÀDžî|IýzÀ;!—rwíÀ<¸£ûó+@OYýÍK@/ªJè\?Ð/níôdÁ?ȑòƱ¿?ölaR*o@œ7^+œ?î]ÝÙ¥¿å‰ÚÔ¯¿ã¡Œý©äj¿äsƒðºèŸ¿ä¼27Š±¿ïþ N¿€´AGNfsrqPMN J2121-6111?ïýÌ
O_?0?;¢§F'?1Ÿ•‡½w?0?;¢§FV?ïýK¶gö?O'J/E«?5¢OäÀNl?O'J/E±?ï«®{ÇÐ?ƒ¿}XZ?…a>Î?ƒ¿}XZˆ?ïî¶G¹Ro?KgÃGòO?aI¸F­Ý?KgÃGòH4FGL J2120.7+4428?î_ffjVÀ<AÏ®)À:?±~'­À;¨iTWp)@æµ+E~@Q*Dw(V?ÇI/ôºQ ?¡M¾ú§%ž?ÚiœÁAS@d‰ÉAþ?ïþj~£ôç¿á+"}¨¢K¿ëáxU|¿á2Åð9¹_¿æyÂr«Ä¿ïÿîbHÊtAGNbcuB3 2118+443?ïô~t¯=¬?Y0'ã^†ý?W¡"§K?Y0'ã^‡?ïÝ@'6Q?†ÔÄ(Šó?q_·äי?†ÔÄ(Šó?î$~Ú:lO?¡¿‹"¸ƒ?­¸\Y;?¡¿‹"¸'?â=¦?v%â#tC|?ŠÚp–}ã?v%â#tCz4FGL J2121.0+1901?ï´YþJÀ5>
 r~À8Šr©jÇõÀ;£ÊÖR‡Œ@¤Î(š@>Õ®Þ]?¢^/š;?­c|ö÷@ÞZ"Ê@
yñßÖ¿À?³mÖVοá÷u¢™r'¿ã‰-°ê¿á|¾ß¤@¿æóBýօ¿ëM³"íbAGNfsrq3FGL J2121.0+1901OX 131?ïûoüöÊ?>ÒÆïìòÖ?B@$×Ó?>ÒÆïìó?ï®ø'Þ‹ñ? D‹®½•v?"AßH]Í? D‹®½•w?ï•?Wy?ŠZ*Ùº?Š°?ê!¿«?ŠZ*Ùº?ïsœÆ­?ˆ=Ø´2Úõ?žqŒg*W?ˆ=Ø´2Úó4FGL J2123.6+0535?¿7{{&À>µÜyÀ9é't1*DÀ<6¶NÜ&@½'ãɾz@
b*Vì?´+®À®l¡?"plN²À‡?àFǨ ž@
ònòÑï? œƒ¿â¨b8Yc¿èž»ýq°G¿â´ˆ"MÝ®¿áØ­«ŸU›¿ïÿânÁŒAGNfsrq3FGL J2123.6+0533OX 036?ïý+öñO?0×i•C?6 Hwå‰R?0×i•C#?ïþD¾Ðô?Cßr&?&û´ðÀè?Cßr%ô?ïæ÷*û(?l/û'¥ìö?iÿÕØd?l/û'¥í?ïøZ!1?<u·Ö"ôÊ?OƗ{9üþ?<u·Ö"ôè4FGL J2123.8-3148?Æ»ú/0žÀFæÄŗNÀ:µkÞuk½À<KŠ·~‡@Ï¡ê ó*@™cˆÕý?Ô]•\s"?à¿-§Ø÷}@0[b&eÅ@^lg1g¿æ"íٌÏ?ïçô÷í¿ë/•XÆ¿ç2UB&Á
¿ïîû.	(¿ìZVÆy÷AGNbcuPMN J2123-3155?îуg'Zs?© ãÜ䉟?¢çɍŠXæ?© ãÜ䉟?ïRҎÆ?¦µMÿP¨?•¥®=g=c?¦µMÿP¨?ëj²–)cß?©bÅ̍È?ÂU5§Zp'?©bÅ̍É?íWm~»!¦?£[_ýlc?µD"
&òÍ?£[_ýlc4FGL J2126.1-3922¿ïç†p§×ÀFþ"ž­Õ'À:µ~Ư|ZÀ<"ú~Ù@ÕôÜ5uƒ@™ñ®-¥?¼A<á1ޟ¿£²€f­?çÀŒ¢8G@!ýŽ?ïý¸ýâïN¿ØL9)y¿¿çê¹aµý}¿áY3BL«ª¿ãùïzv¾£¿Ò<ªÏ'AGNbll3FGL J2126.5-3926PMN J2126-3921?ïýÓÉÁæ?1"Âz8ï?3a±ðÍ?1"Âz9?ïýîˆÚdñ?H¾Ìª­î?0‹¹,Øsâ?H¾Ìª­î?ïëú¬ŒÇ?j]Ï1yù?d€Ss8á?j]Ï1yå?ïõ6äÓL?DF'QÇjý?Uý'6Yl?DF'QÇjì4FGL J2126.3-4605¿ÄSš7½3ÀFÏG0@9¬À9kæ'øÀ<5/Ùâ_@\XúÂÿD@Aà?pXX?¦ó5—;›b?¥P(as'?õõ+á/Za@Àw¥("¿ÍßÈýà@¿ä/D%ɾ%¿èèSpÀ\|¿ãOCÕAæT¿ë`›KJ.¿ïúÕô"»3AGNFSRQ3FGL J2126.5-4605PKS 2123-463?ïþÂ~ž_•?dÔM±Cf?#تÍ?dÔM±CZ?ïý½¸bmþ?L…U•˜?2<ìß?L…U•˜?ïåyÄ,€Ÿ?modj²Œ`?j†;Ó`?modj²ŒP?ïÿùú€An>Äi˜ô>ÈþúMín>Äi˜ù•4FGL J2126.5+1842?摩Ú|À6m»{k±)À:ÏáÕr¼À<wª¥æ¯@ 4‡†Êµ@ÛÄÒ,ˆ?Á"AÞÇ¡¿¢|ÉCI?äMÝ|è‰@aŠžÿßõ¿ëä¡Ý4ú?ïÿÁeÖt¿êÁj=¶nç¿ÉŁÿÉú5¿á*«ýI¿àaO`eprAGNbcu87GB 212407.5+182753?ïýSàŸ=?8)Os~?7M`ûr?8)Os¸?ïýìþ:)?J?ÞÈw©¨?0˜¾.º×?J?ÞÈw©"?ïà{&Ҍr?r8=8Y?o"Ù-sÃ?r8=8O?ïïã4Ó.?Qň)f?`Ë,ÑðÎ?Qň)g4FGL J2127.6-5959¿À¡Úê…(ÀE=¿H˒À;X?½…1-À<Üdçá%I@ š-hC
l?üuãTΎ?Ë:'C:è?ÃÃú€º$ª?÷ځNš@""¯ ê?ïîy$¯ò¿í:䜸2?ސ'¡»ý¿àʐ¢Oοåñ6;%¿Ñ²'¤\ìAGNbcu3FGL J2127.5-6001NGC 7059?ïýAJþç?:T{yâØB?5õ¯ˆËó?:T{yâØ`?ïýãî<'?FÍ[øNª?0àŒhœ?FÍ[øNŽ?ïØÙ
Û­?x=3žîæ ?sÀy)ž?x=3žîæ—?ïÛkö'L?`iò¢x_ü?rqʶ٪?`iò¢x_ú4FGL J2127.7+3612¿¹A5
]À%ùÁø]tÀ9Mo«‰†&À;ËüÞ1@Ês×K?üþ_·¼^?²a>‰R¥?ÀN®ä¯l•@¨!ò™0@1<ëج¿ÎÍÅÆ[¿Ùú$‰LD|¿Ø~¤`GŽ¿ßŽ?ÒþÀ¿Þ4"ý#Ö¿ëá& þ'ÃAGNbll3FGL J2127.7+3612B2 2125+35?ïùk[ÒÂR?Faú·úé??JR´ö²Æ?Faú·úéS?ïù0±ð…?i¤»mƒî?K=9È=éŽ?i¤»mƒî?ï¢àéHY?‡=búÍë"?‡GÅ­à)Ò?‡=búÍë™?ïáiŽ·<?T¶ø5èrž?n–þqHÃn?T¶ø5èr 4FGL J2130.2-7320?±ÕÖ՟¤ÀBmß 'áÀ;JòÌ:֖À<Äô,'@É{ôíþ ?ý=¨!ò™?ÒáÍdø'D?Ԋ\¥Gw¹?ø*²ái<@8ô‹(?î˜32\sž¿íè†1		?²|Ç£m-¿ækµÆ 
b¿é/ôq¬¿¼%p§ÝÕAGNbllPMN J2130-7325?ïçæõہ?c¦™8y?hå
$€?c¦™8w?ïüŽïß]?T"µë:?;ˆ‡Þ?T"µë:?îÉ5–Œ]?–pŽZmg"?£l¦—>JI?–pŽZmg"?ï×@	vG?bå%Nûôí?t_ùûD܁?bå%Nûôó4FGL J2130.4-4241?ï(Ÿ,íÀGUž™ À:•êњ'çÀ<t&"»@G6¢0—@Ð#éê?Æ?a>ß8à?›ÕW	ý?ø§°³'@Ù{´Qy¿éæÍÿÒ³—¿Ö"š.¿çå¢'<¿ã8?ân¿ïû›÷Ì«¿ï=I6ª·AGNbcu3FGL J2130.4-4237SUMSS J213017-424319?ïþUÓÕíñ?1Æóâ^è`?*¢Â¡ å4?1Æóâ^è!?ïþ&øZÿ?I"&Fa‹?-– zP0?I"&Fa¡?﬎J[Ž1?ƒ¯o¶?"Ümism?ƒ¯o¶?ïÿéªS;H>à¢י>æU¬Ä¶ÀÈ>à¢ÕÊ4FGL J2130.8-6623?ïü‰•_ÀD È`VíÀ:@.A[êâÀ<Äa¢—o@1O¥"´Z?üØ´|sîå?À'ý]¹C®?ähY …F%@ }(®tòñ@ÿ9Cm"¿é Û!¤??êìȀ6ò¿Ò//bÄw¿é.äïÙA¿ín—ø¯©¦¿ïýÑò¦{)AGNbcu3FGL J2131.1-6625SUMSS J213038-662356?™_6ÒZ?©õ¦nºò?ï5Ioçï?©õ¦nºò?ŠœTp	¶?'-wyÀié?®=ûÚ?'-wyÀié?¦ÏíåP?šHÛô" P?î"&ñ«?šHÛô" Q?Š@ì"\?€"Á¼Õ›Ò?üOwÓ?€"Á¼Õ›Ñ4FGL J2131.0-2746?ÚlEØ$ôÀFì×à&EåÀ9‹‡T¸À;ìh?"zN@3úÑíÈñ?ùóúˆÇº>?²¼;7ó?¿	Hþ÷l^@+ý´Ì%@
§&5ô®"?ï'v Ùó?ÁDµüü•g¿ÉΆö©À¿ÜZŽâ™¿ØÇÓ~AÏX¿ãcs¢¡AGNbll3FGL J2130.8-2745RBS 1751?ïﵸ
Û?d3)™ªÇp?`JGìò%?d3)™ªÇr?ïí
±ôx?"fk0;?bõN牿?"fk0;?ï–NLŒÄ?‹FÉ÷`ð?ŠllÜÎýG?‹FÉ÷`è?סּSƒ¸?p®1îDŠœ?"Ÿ«?Qû?p®1îDŠ•4FGL J2131.5-0916?ïэ¾&ϽÀCÖ@|ÇÑ»À9¥
œ;5À<%Åo@	_	ç?ÿÃnÙј?°gÆä*Œ?fœÏŸ‰'?¹ìÒў˜²@
-:×ÂI;?ïsÿi­¿ßD¦âÔ¿ãÿ•g0¿ÚE¿'Q¦¼¿á•Ÿ¤u•®¿ÇôwáùþAGNbll3FGL J2131.5-0915RBS 1752?ïþï[éV¥?Z5ÿë´?!
Aj•Ç:?Z5ÿër?ïþœ¶‡*Z?AB‰€^ûŸ?&4—ZOÐ?AB‰€^û–?ï÷''yÀ?YÊMŒ*ip?QÄÜÝ~'?YÊMŒ*ih?ïükË?hõ?.Y÷-E8¬?<¡¦¸S\?.Y÷-E8"4FGL J2131.7-2515¿€ÏQæ¤ÀF»F^‰"SÀ:YìÝ
Œ°À<ZSÆP±É@ nYÎÓb=?ûÈF¥Ö¾¾?À¸ô'ڏƒ?¿×´ÝAäý@ÅzxQJ@iÂß84O¿ïŽI9.õ·?ê)¯[¢¾¿ÙÁa3Ϳע."'AÜ¿àÿŸY¿ÕŸç't1AGNbll3FGL J2131.8-2516RBS 1755?ïñ1ÊÇï(?^ꁯ­xv?]œjp!®[?^ꁯ­x‹?ïùâ	H……?f~Ò¦÷
?HwÚÝéíý?f~Ò¦÷?ïÖóáµÝ~?xÒзM?t†%A"?xÒзM?ïªÔû÷Q?r"&Ëę̂?…JþÁ+í?r"&Ëȩ̂4FGL J2132.0-5418¿ëp´&™äÀFliƒQX¸À:	²Œ¯¦KÀ<jńÙîô@Mä@Ü¿@G?Y²#?¸y€Ÿwª?³ƒS‡ªó?ø9ߊ>²Ã@ó–ßU§?î+|…Œœ[¿áEäEVJ¿ä^_[Û¿æIøÜö¼¿èñÒÀ¬­ó¿á_L@ËLDAGNbcu3FGL J2132.4-5420PMN J2132-5420?ïû8³?;´J#@œ?CÓ¿Á3›?;´J#@{?ïý³Î;¬?MÜGÙøÙÚ?2aŽ"›?MÜGÙøÙ·?ïÙks³Sì?qÃ%8*1?sJF&V
%?qÃ%8*,?ïúÿkšc?1ñNߟe?DSіrü?1ñNߟU4FGL J2133.0+2610?ÁA¹C0ºÀ2q»à~íÀ:×Üßi‡ƒÀ<?‰›ár@ù¨çj\ë@¯ŠÄê€<?˯æ8óg?Ör$u*Nˆ@ýæJLT@´²@¦(?Ñ
8þyB6¿â¨˜é_¿çMFkE¿äã¼gú»¿ïþ€¢§µ¿±Y¯ô¤ØAGNbcu3FGL J2131.5+2605NVSS J213252+261143?ìòúüad?µz –2¦?¸ox(ôã?µz –2¥?èT®Ü?ͪsí?ίñG³ô?ͪsí?çRbÍ¢yo?²ú5K£K?Ñ[:d»
"?²ú5K£K?äΫÒöãÄ?²£ûEÀMz?Öb¨Z8{?²£ûEÀMz4FGL J2133.1+2529c?⸷䧚KÀ2óNe¾ ºÀ:«ï}Ѽ÷À<j"l
ë@ ¬³Ho-?þȼg#ûˆ?Å'Pǘ°?¤Pl ‡‡?ã>Ÿ&Kn@û©Ã2o>?ïúޝڛí¿×Ô¿?E-¿à£^Caÿ¿ÎR$zˆ²A¿æ»Ê`áÂ'¿ÒƒSœŠ9ÕAGNbll3FGL J2133.3+253387GB 213100.1+251534 ?ïþÖ)Xè#?¡Rô!—/?"jq}Å?¡Rô!˜?ïýÕ½<:?M!GVŸ?1R+}ß?M!GV™?ïô…ê÷pf?d><n-_`?Vô*8.?d><n-_[?ïì!¡¸ëf?Qوôe?cÞ^G™'?Qوôe4FGL J2133.6+1439?Ïë$¾21ÎÀ:d6†¤ÊOÀ:½|·¸À<" ()ö@@Ã]NÞ@ךCÅ
?Æü7ž}¿®$=®X»?äµÎMÖL¨@c']çç°¿âøâÕLοë]
Œ°}¿å'z¡0ç©¿æ9Mß0ýy¿ïæ¸f
{¿ïÿò> wAGNbcuMG1 J213339+1443?ïÿRg¿6x?"ó¤)m
?³0ëñ?"ó¤)mO?ïùtSÓÁs?lEìE"?J.°°ú:s?lEìE"?ïámQ_?sH˜H膾?nâr'® y?sH˜H膸?ï÷-.ÚÑ?AÁå/`?Q¥¢J]ß_?AÁå/_ô4FGL J2133.9+6646¿¯ïg^÷$Ë@%ù
{é…jÀ9Wòw@ÝÀ;òd\ êÇ@åÄ[º@èà(Ê$?´"54Y©?µ@b›«—ž@
Ú\ˆ–@½"NXӁ¿â<kU¹où¿Ñ´ådô y¿ån oQ¿Ö'°œ?':¿äé2(q8R¿åFÆÞvB|AGNbll3FGL J2133.8+6648NVSS J213349+664706?ïüÞ£·—÷?4:ÿ[že?9
âC@<Þ?4:ÿ[žE?ï÷Œ×F«?jä°Ðÿ0?PæQrz¨_?jä°Ðÿ.?ïè"YN%?n2ç÷•UD?gl¦±øÛ©?n2ç÷•U_?ïë£Lw?Sdb‰‹•?d\³ˆëá"?Sdb‰‹‰4FGL J2134.2-0154¿àÛy"¾hÀBDzd×ñÀ9àR»Ž·À<I—"Ç@Ò¤e¥vG@DfBT?ªýd©g?«èž ¥¸@=ÙÂ~•1@‹–'(6*¿ÖóünñO¿ãaþ»Ý;¿äîvjÀh:¿â#•›Þx¿è • ãû=¿âᙹzAGNbll3FGL J2134.1-0152PKS 2131-021?ïýX?õ?02¬<È«?5?^Wƒs?02¬<È«?ïý­¾mƒU?Mb>ÇBe?2'"åRÚ?Mb>ÇB:?ïà¾ÓÕ?sg}y?oóâA,*'?sg}q?ïý¸º±Æã?&½d.ϛ?2:*qÈßJ?&½d.Îþ4FGL J2134.3-6511?ؤƒ5ö+ÇÀDc¡À:Ç+×_gÀ<aýõ}Æ@Zt¥™W@Cá8j«?Ðe¦Ñ?•ÿ¥DÑó?·™¿¯,þ¼@ª7îý`¿ìÒÿõ5¿åk›#ÝTÚ¿àm>K?D¿åNìóà¿å°¨t'ð	¿ïîW–¿Ê†AGNbcu2FGL J2134.5-6513PKS 2130-654?ïý'f.à?0ßJ1ÿÿ(?3ìΈÿŒ	?0ßJ1ÿÿH?ïþq•}pË?IŸ…˜ÞËg?(æ¨(ó<Ö?IŸ…˜Þˀ?ïߗ}ξ?t_DQ@"?p4A öü?t_DQ@"
?ïúÂ$¬Ñë?7TÙl™è¼?D÷mL¸Q}?7TÙl™è²4FGL J2134.5-2130¿ét|û±¶ÀF‰Mçê_…À9xˆ3?ÈÀ<¸_W~l@†Cmqs?þÙ²"ý[
?°Ï¹Wf?²Gšs^F‡@¨Ÿr÷@)0Ôßù¿ïëC_Ñ ï?ïÂîþGn¿Þ¨èèŒF¿àcª2n¿á½?[_¢'¿à*MTAGNbll3FGL J2134.5-2131NVSS J213430-213032?ïþ'dYîj?$žgœ©=Y?&éºa`?$žgœ©="?ïü°»C¡t?][û7¥?:z%âôa1?][û7œ?ïË© 4ªŒ?}Œ-Žʅ?z+/媺½?}Œ-Žʄ?ïôð4½?MŒ‰Ó¹?WÜ—à†Õ?MŒ‰ÓÊ4FGL J2135.3-5006¿ØcF'ô¥ÀG3)¡¹ù‹À9-w9ó@ÕÀ<AÞÌ©'^@])DÇÛ @'bå¨eå?¨µ#§"Ç?²Ë›^ëÈ@"˹§V@_kó™d¿Ðð÷¹à`þ¿áîÅæ(¾e¿æÔ²¡¨\¿å§­ÞÊü¿çȈd½ïº¿íÃz=³¿¶AGNfsrq3FGL J2135.3-5008PMN J2135-5006?ïý˜*qV?0² &Œ-¿?3>¯uN ?0² &Œ-"?ïü¶'*6é?Y¦)høÜT?:Kv®H²¯?Y¦)høÜN?ïáÎHIíæ?l>6¤ñšˆ?n1·¶Ù?l>6¤ñšˆ?ïö™r8¹¯?D補"ˆ?RÍŽŒ¢?D補""4FGL J2136.2+0032?ÑV°YÜÌgÀAÊdÂø7µÀ:÷Q۔çÀ<DFŸ@2΋hÔU@dZ˜Ó?ÀüÈŠrà?̙}jº@ FÇd®@ج8'¨f?æø¾&@Ü¿éòÚ/­m¿ç» !³ƒû¿ïÿùµc#¼¿î¬¢ŠÙã?ïù!bü$AGNfsrqOX 057?ïý×?%
X?3ª¬×Ń÷?1Fו?‹?3ª¬×ń?ïþj<g?Fý¦¸þž¿?/‰\9—?Fý¦¸þžÅ?îOèfÅrÂ?™p¯4¤]?«y"¨ÓÇ?™p¯4¤\?ïýjƇ£?*ŸA(.Ç?4©ËÂçG?*ŸA(.è4FGL J2136.2-0642¿í¬bú&ëµÀC¼ƒÛÂ3À:çž?ñˆÀ<l*YoÞ@bâ'']@6¹£$]?Ä%W'"(n¿ppëGÀF@ÃÀ0²$?ïÿ*þ~ð¿é$žoí#¿âŸŠÿøÉ*¿ìCžOá¿£¿Ïg¿Asè°¿ïÿüñýAGNbcuTXS 2133-069?ïþ4˜/à¡?26Š©ÝŽ)?,¶}õç]?26Š©ÝŽ?ïýøN:^G?G½ƒjH0¦?0=Ž-
ÅÇ?G½ƒjH0¶?ïˆD*V›ë?…>8Gß?¿?îõjYé?…>8Gß?É?ïöØO[–x?FoñÃ{S?ROaHÓ?FoñÃ{U4FGL J2136.5+4259?Ë@æç"QÖÀ:î}÷|¤À9Ê3°0´ÔÀ;´SFÎñj@RŖøƒ@Z—ÆZÂÄ?À† •÷£?š¦ÚtÖÌ?×vC=ÂXU@՞ñGU¿Öܱ±¾S¿äÁ/	ØÆÖ¿é`›š›ø¿á;4‰tˆh¿ïÿûB«÷¿ïX—;ˆBAGNbcuTXS 2134+428?ïþÆèV–?2Dq'j¤[?&ó'z–"¹?2Dq'j¤©?ïþÚµc'j?JhÒÿʐ?"T©ÇÙcž?JhÒÿÊx?ïkPF¤?…ŠÅuD?'•þ÷<K?…ŠÅuB?ïÿ¶"¥¥Â>øô®VN?[–L>øô®VIH4FGL J2137.4-3209?ÅOQµë¿ÀGób¯È°À;0vŒNW|À<®Úb·…=@ _Nã<û´?û0"|Ñâ¶?Òy˜\؞?Ìç±"_É?ýÚu+ü@—2[%@¿ïÿß´0Õ?ïüÉ_o¿ÖC™J~(¿ÖÜL|Z¿âi[
lпíýZ~{°ûAGNbcuNVSS J213726-320755?ïý—˜ü?43—¹H.?7»C?Ø"W?43—¹H?ïû`æýîœ?cÍ)2$pq?B|dEŽG?cÍ)2$pk?ï¿&µÕu<?}‹‡ƒÅ™/?€6RŠ¢±B?}‹‡ƒÅ™-?ïÞq?`Èp…4ÿ?pÇxðwrC?`Èp…4ý4FGL J2138.3+3556¿ïå3	•,¢À(w°ËæÀ;hájéƒÀ<}~´;@ ß³î¯u¤?ü±*ÇC ?ÎØLÈ/¯?Á>Þwšj?î3ÓÃt^@î¹[«Í?î½cm¢¿ë±K1Vº!?í˜{Ò7ñ¿ãÞ¢ýñ\ú¿×·†^ÔKÇ¿Óu3=šiAGNbcuMG3 J213809+3553?ïýí0?*ÿÎ7€¢?0‹K&y4?*ÿÎ7?ïýŠS¨¿©?Qœ´ƒö̬?3­bº¶"?Qœ´ƒö̲?ïç)u_Rå?iaŽîCO?h֊ ­Y?iaŽîC??ïÛ¼æL;?eåô!«Ñ®?r!òŒÙâÊ?eåô!«Ñ§4FGL J2138.8-2055?Ó¿6™T¬'ÀFì¿Â"OÀ;6ÍòfºÀ<ŸK·Žw'@!N¦.Ð"?øî"ã)/¤?ÐÍ>aº…?ÊÓ=ª/"ì?ü)T!ÀD(@ªL›,¿æ¯˜Ÿá²¿ä™Dàá6¿æ9¨bŠ8Ô?½)6@j£¿æâ
·'$¿©Úó+0ZfAGNbll2FGL J2139.1-20541RXS J213852.9-205354?ïúÖ2,*m?<_:Ÿþt˜?D§7OVL/?<_:Ÿþtœ?ïûÉO0{?YJ"¢È;?@ۚÃ>r?YJ"¢È-?ïÂ¥YüA–?{àKSzl?~­Sß47?{àKSzg?ïêºã•ž?^4³¾@«¨?eEjðbQ?^4³¾@«³4FGL J2139.2-2214¿ïÎÁ¼wØÀG+'·þÀ:½-Œ*EÀ<f'}keª@ÎuÉ/ß@Ӛa?µø?ÀÉp·M3º¿²¢Øü0?ÙeèðïÂ@çØŽZ ?Èòdvw*¯¿ì=èîÁ¿à_$ù´Œ¿åœí ªD¿ïøÊ¿˜‡¿ïÿþ½à ¿AGNbcuPMN J2139-2213?ïè>¥Õ
"?nTv°i?gÁZ*òkë?nTv°i?ïÞà'¼œE?Š™p"Ï?p¾¡±Þ‹?Š™p"Ï?ï55á÷ؤ?ÎKò8JÙ?™YCÁëW?ÎKò8JÖ?ï¾¼?pJÓì`ö?€x~øÜJ?pJÓì`ó4FGL J2139.4-4235?ïƒ^+'N^ÀH*løQÀ7¤P«>¡À;=€Íù¦@ǘ°eŽ?þÞº))?•="½5øW?©(÷"¿P@@#L]¦¤D@Æu)LÕq?¹³V.4ñ¤¿Û:ð@ð¿àÈÎ:‹I¿Ýó§ªS¿än'?ßéà¿áyÑÕëYAGNbll3FGL J2139.4-4235MH 2136-428?ïÿ>zv³Y?QAHŽ-?0±)•H?QAH?ï÷Æ)ÂF?hJ%"ìÑ?PsÁ¬{vÞ?hJ%"ìÍ?ïÚ]KÌÂ?|vŒnÖó?rþÑZžù?|vŒnÖö?ïÿµ·Á>úª`q¯/?º¸Rl
>úª`q­4FGL J2139.9+3910?ç5büV†·À$$ƒDÃ~À:^íLŸÀ;íGô‹W·@ܹ©.@¦ÜG©ã?ÍþAŽë–?¥äìź?׌4á߯@‡P&3¿ËŽ²µÊQÈ¿â÷Lg·Ÿ>¿ëõTáä·¿â?°"—©Õ¿ï÷d?ð…å?ïƒ/ÊÈæŽAGNbcu3FGL J2139.5+3919B2 2138+38?ïþ¢ò¸â?0)–îð?%ßàÔqñ°?0)–îí?ïóç4`ß?yvŒµŠÇ^?X1ӗ>>Ú?yvŒµŠÇ`?ïk='gÃ?ƒäæå?'˜M³çŒ?ƒäææ?ïø¶Ø¹	¢?BØ/©)Œ?M$ÙwJ?BØ/©)…4FGL J2140.5-6731¿Ö€$0èCÀDGë¿×À;&¸Lã¢À<ߺmN·ô@Z=~»œÏ@8ÇAr'?Ô2È?ïí8Go*Z@%žÀJ‹@uçâQï6?ïØB¡»&¿­}õ¤1x¿í…B>éÊ´¿ítÈ~ßY¿ïü•è41`¿ánß{ûùáAGNbcu1FGL J2140.8-6743PMN J2139-6732?ïÝ7ܓ²?ƒhôˤB?qd¶'Y?ƒhôˤC?ç"U¸]Q?Ñ°±¸"C?ÐÙTE]É?Ñ°±¸"C?è[ãXlæú?³¯V"9wj?ΐržLd?³¯V"9wj?åÚx©Dœb?ºH&6½È?ÔK­vÇ:?ºH&6½È4FGL J2141.4+2947?托KŒGÀ1/pyåŸ,À;»Üº€šÀ<u<;±'@u¦Vkq"@d˜Þˆ¶ó?Әíùþ?цÑ`/j§?úûs5X§@µ‡¼!ƒÞ?ëQóþ¿Úž+Cû'm¿Óä/à'S¿ç\cáPè¿á÷‹òç鉿ïÿïÕAGNbll87GB 213913.0+293303?ïõ1'»†?Tæ×	•°?UœÛ؈ö•?Tæ×	•¼?ïüÕ8¥Îº?^1)ü1vð?9V:ъ'+?^1)ü1v÷?ï$
>Ó+•?'(&‡QöA?›~¸%šf?'(&‡Qö>?ïÇ@>ó#Q?g-'œtÀ°?|_à†nWU?g-'œtÀ²4FGL J2141.7-6410¿Ô€˜`WõÀE#KßÒcÀ8;"‹›˜À;ÂûB+»@Ðڌþ×@ÞbV6mz?œ5Qßµ?ºIؼKV@Z…‡"ݘ@ÇùZ"z?Üŝƒ‰¿Ýïâ+XÉ¿åwŠ~Ÿ¿äø¸BÒ¨¿éKʾՓE¿îˆŸ@¢‡AGNbcu3FGL J2141.6-6412PMN J2141-6411?ïéûaÞ6?c˜æÐ+ïÔ?fž!êÊ?c˜æÐ+ïË?ïî"P"¼'?€›Õ.w–?al¯ÝC|R?€›Õ.w—?ï¡pțñã?…ÛòðÌæ?‡£ÍÙ‡)?…ÛòðÌæ?ïþـnà?9›"ö'?"gù!úœ?9›"öo4FGL J2141.8-3727?ï"öª÷=\ÀH‰GyBÀ9¢âž43À<F!*òó@9f­6Z@ÞÚ4"\?±Ë¾.ú>u?šwA] ø'?å	Ö¾IÚ@#ƒÊÐH¿Ö*¸¾«¢¿æá_¿æϋXŽ6¿édk"³Xˆ¿èt·,Q—¢¿ðAGNfsrq3FGL J2141.7-3734PKS 2138-377?ïÿu±Šo»?°%¡U~?Iβ{P?°%¡Uú?ïþ[À"?G¯ú'ºÜ.?*CþN¦Ã]?G¯ú'ºÜ?ïã$›Zd?jOXÉ!?l~Ûd¥œ5?jOXÉ!"?ïý†Õ¯q<?(b»Vð/¹?3ÉR"vX?(b»Vð/®4FGL J2142.1+4501¿î_7I¡ž—ÀØ×à&EåÀ;	r£‹‹À<|CécÜ@ תU(¦g?úÒéF€?Ò¸D‹ÑZ?Ѿ ™'¯?û'fŸqJ@Þ«T4¿ïר¦Ó?ïû@Ô磿åʧ=Ç
쿼Gmý´¿ãCcaÏ'ñ¿ãтÿyGjAGNbcuB3 2140+447?ïüjŽ ¸?5åÎj+.Â?<«ºú;˜?5åÎj+.Ã?ïú?'ä]
?gEoˆ¤?G´n‹Óð?gEoˆ§?ï±ùÍYÅ3?'ÄÓÃ(ík?ƒŒ©Ž³c?'ÄÓÃ(íf?ﻼ·…?s嗸fÂ?9úRê?s嗸f¿4FGL J2142.4+3659¿Óáe†/VQÀ(Ïå†6À:x(E™gEÀ<Rñ¹_ä@ Äbr'æ?ÿ5Hyd?À]ÚPÃè?"/Àô½å?Ê@±ád"@»ti3uM¿éçkÅ?ïýTõ$Ú«¿êí¢ò(§¿ÌžnÀ}¿Ø`ÈðŸ:¿ä2jGâAGNbcu2MASS J21422658+3659481?ïü¬¶é?:ýŠ‰Öˆ?:šOßµ¾?:ýŠ‰Ö¦?ïýӹɧ?L½0êå`*?1g¢1²ÒZ?L½0êå`?ïÙjâBš?vl–J
~?sJŽÞÿ2¡?vl–J
|?ïñ³žA0?PT±'fû.?\™ÂÃ}¡û?PT±'fû84FGL J2142.5-2552¿±m'˜lÎÀGý–áXuÀ:h˛teÀ<nÉìG¼W@ªü~ìC@Çùä]K?½Ùz|rí?À=
w}:@
;ƒcÍ@ãÃ"´?æ'ú㱿×Pâp£K¿çV±v/¿Ö}ê;ž¿ìÑý"ÕíÞ¿ï¥è\uKÜAGNbcu3FGL J2142.2-2546PMN J2142-2551?ïñ­Î?Z§ŽYõ^
?]ûè¤cÍ?Z§ŽYõ^	?ïýԃïrF?Mßbå7¼¾?1[à"mÖV?Mßbå7¼â?BÇ{×?‹	~…¿€Œ?ïN!
_?‹	~…¿€‡?ïù£=-͞?8†—Hie§?IsHɈÎ?8†—Hie|4FGL J2142.7-0437?é}y"ŒÀCä"&þrÀ:¿)h¯À<ẕ@tÀ‡o@ö‹AèÜ?ÈÛÁœÂîÓ?§®šÑÖL?ß¡/$°¹q@ÍåûŠ¿ã:;e0ÜA¿ã¤ñ@õh¢¿åõ²Ÿ$¿á%sW±N¿æ¨ Åó?¿ðAGNfsrqPKS 2140-048?ïûoôYŽ?>K¢Es•?B@.™½Âª?>K¢EsŒ?ïûi‹žÌö?\õœÒ-Fœ?BYфÌ)m?\õœÒ-FŸ?ïÛCþ@Æ$?sM¹bIò¬?r^ߜî ?sM¹bIò¦?ïêØÃÚg?T¯énvØ?e'<ÿ%˜?T¯énvÓ4FGL J2142.8+1958¿¯‡3püð'À8c`9%»{À;°)(vÀ<ŠxËøQ@!q¹7C¹?ù_=?%°?х™ž!?ÈA÷[ÁœÃ?ù®} ½ê@	XfŽTl?渘B+ž"¿ì%ôïo¿ÄÝ·*Ï¿ÍØçø¢=­¿â?`A^D¿Ê4³{mÂAGNbcu3FGL J2142.7+1957NVSS J214247+195810?ïÿ,IMƒ#?Æ[š
I
?vÖO›Œw?Æ[š
I´?ïþŒ¤­aˆ?B­Óö?'5µ)çiN?B­Óö	?ïæÆ£J?p½ƒ(+Ò&?i9\µíë?p½ƒ(+Ò!?ïúWþ0"?6«ÿõQ÷?F£Œ=¬U?6«ÿõQæ4FGL J2143.0-5501?ã0û»ohCÀGh3Æ*À:·"òsOƒÀ<lꭈcç@jŠbo@…ËÀ]?Õ¦"»ë?ïÿšr¦ç@Ĉ'ðà¨@gIh~¿³Åüà!#¢¿æ¦²¡¨[Ô¿ïþdõM—?ïp¥ïé1‡¿ïÿìIiÖ]?ïŽéõÒAGNbcuCTS 0561	?ïÀÌÅN–Ê?'ëP¦z<b?™X´šÏ?'ëP¦z<c?ì#Þº‡ý?ÍÁ–EÈ
[?¾á
+ÇÈ?ÍÁ–EÈ
[?ë/WGGŸ?¬–ρµ?ÃB£–âá?¬–ρ¶?í'ø­²¤­?¸0ªšãØ?³è:'jڕ?¸0ªšãØ4FGL J2143.1-3929¿ïH}¸AsÀH¢ÛߏG0À9õƒ.I½À<W"4$Ê»@´çër@(¯œ:]Ê?´F¾?ì)4¿xÁ—©CJ?Ÿ±m@ôÙjM?ë.Áÿ"JO¿ÛWUý7£°¿åJàc'†X¿á'K3Úøß¿æ!ú[{PÙ¿ÌËc@A8¯AGNbll3FGL J2143.1-3928PMN J2143-3929?ïþ1ÞÇ}ë?#×yèqQ!?,âˆ!OB?#×yèqQP?ïþá°yß«?=œ¿R›å?!äøb[È?=œ¿R›§?ïò§Ïq›¾?bt],C?Z°aȃ7?bt],X?ïÿ#­üÅb?qµàB?Š@gSߢ?qµà@û4FGL J2143.5+1743¿ï«"õÊÎÍÀ:غ@ÙÀ7gþR€ÖTÀ;iÍ9VÍ@ù§>Ê@šz…\!?5…¦{2?£gQ×kâ@
…bÅÇõÍ@^'Š]'¿Ñ±U¢ô·"¿äâaÿÏY¿çRºýÂc¿åÉVAU¿è}ÿºà¼¿èÌ{n5gÁAGNfsrq3FGL J2143.5+1744OX 169?ïþ	°T±ê?+Ûâæœ
S?/dú´áXÆ?+Ûâæœ
F?ïøEò£Úy?e…±"Â*Å?Nè5p–a?e…±"Â*È?ïkpº±¹?3IÄ?''è©Üˆé?3IÈ?ïû<ÑŸ®?:K—"¼?C
ˆ¹LÂ?:K—"Ô4FGL J2143.9+3337¿æ_–Ò׏À-s¡ƒrçÀ:ÆXaÀå8À<iï¤h)µ@ aê»PR?ÿÑ*)Ÿ6?ÃZ°ûŠûF?«*n­+È?êpå^"
?ý¬ó@T¿ïù¥þÐ¥?ïÿû˜'2¿¤ÉlßÁ
¿ä²¥~Õ(¿áy‹X࿼ÚÝܔ•úAGNbcuMG3 J214351+3337?ïýKÓþ
Ú?2p×±$d$?5¡`'6œ?2p×±$d-?ïøpÐAdä?ixü'É"?N<¾úlhÑ?ixü'É"?ïLjZäx?~jˆ¢q·à?|;ùҍÃx?~jˆ¢q·Ù?ït…ÝX??€õ˜Õ4?'oDTø?€õ˜Õ44FGL J2144.2+3132?ãjº3'À0M>Õ'å!À9§<t$•À<+ºõ3ô#@S0 U @ƒ¼ûžqp?³êoJ×?­Y2Ý^%¶?ø"c¯ÒÁ@
<'A¹2ç?ïË}ÂM—ã¿ßAݨ[S¿àá–5df¿ãªŠLõ|¿Ùʊ<ÚPï¿ê) ¡`7AGNbll3FGL J2144.2+3132MG3 J214415+3132?ïú×WÛs?B¢-3>Õ"?D£' '1C?B¢-3>Õ?ïýO›Æ³Ù?L~)ð'V}?5ƒ!Êa)@?L~)ð'Vs?ïã–Õ\J?s;GþJ‹\?li*£µ€Û?s;GþJ‹`?ïçWõÓºx?S<#B§?h¨
,E‰M?S<#B©4FGL J2144.3-7802?ê9†yAÀAuäõ8&À:l&ûíLÀ<£u»n@ôí}F}@C…%nN'?ÓÀ£~tÐ?ÐM`…ü¯?ödŽTÁù4@
3Ï.Pö=¿äþ÷Väd¿åv…}'âž¿ì"+
oÆ¿ïüë"£C?ïÂ}h‹…¿ïŝù¥žAGNfsrqPKS 2141-781?ïÿqìˍ? âÐÌ;5e?1ÂfŽ0¤? âÐÌ;5ô?ïþ›.Ý?MÕ·`m?&Mb.f¶?MÕ·`m1?î"çæLů?™–'<÷Œž?¦±›3¥?™–'<÷ŒŸ?ïÿ¬iœÃ?èÅL'?å˜þuT?èÅL'ž4FGL J2144.8-1817¿ï¢Ð£<CÀG)ayWÀ;h¥IÑjÀ<ºqÊG·O@ ä²hG'?ÿaueݪ?Ì r}ËÞ?uH¥qzQç?¼ßŸb±P@vO[‡æ¿ïýQßñ—²?ïÿÔÌuŽø¿â
Ò¡"$¿æ¢f&¥†7¿µtSäوó¿â¿ý¡UûŠAGNbcuNVSS J214442-181801?ïÿ;»8'?.à'`î<?ŸH˜û?.à'`íP?ïýû¢†?UnÑ̺™6?0"ï;Îÿ¹?UnÑ̺™7?ïÇïcP×?}ýBÉwe?|sNW"š?}ýBÉw[?ïûë»;Ÿ?7+åãž×Æ?@Qƒ‰?7+åãž×¼4FGL J2145.0-3356?ÜÝN2µÀHÐGG"#À9HÆBoÀ<÷ïF4@֒­Â—@O,e¹˜=?©-ÝÞÂî}?¾&•Q¶@³w[0@»Õ]jo¿»v|3,RC¿Û–H¬A<
¿ãø#B$g¾¿æhH‰͟¿èÍÃØ1"Ý¿æ]THÏAGNfsrq3FGL J2144.9-3356PMN J2145-3357?ïùIÈo?Pï|mÛ]I?Jۇ°ÞA?Pï|mÛ]K?ïúˆû#a?`*ûõ]Ü?Eß r}?`*ûõ]Ý?ïuÂD¾£?‹]É&¼?'Mç·h+µ?‹]É&¼?ïþÄkÖòP?y­ãÔ´?#¹BÛ}?y­ãÔ4FGL J2145.5+1006¿ïïÚ²L]¯À?ŒÌxéö©À;^.†%HÀ<§Î_ª@!í9Y=?ûY'ÿ?А›ëÙ?·Š¼+R?êϔÈy€õ@.-%Òø`¿ïÿÆߢèM?ïì~Bûþ¿Úd\åX¿ÚÇýsޟ¿Í–ÿöÅě¿ßôâ?¥²AGNbll3FGL J2145.5+100787GB 214302.1+095227?ïÿÓL½ÛÍ>õP?…}ì>öY¡÷6>õP?…}…?ïþd®€n‰?LÄ9_LÄ?)µùlÜ?LÄ9_L»?ïó:̃Hè?céÞ´ü?YŠfùn-Ÿ?céÞ´
?ïüèãî™?1Áoñ	:?8¸çˆ‹C ?1Áoñ	44FGL J2145.7+0718?èGӍIÂ(À@´Â	$lÀ:µmÖPÚÀ<]¸"Üû@ q›#òÎ@Ñ|^?Åçþ×`ú¿•vFáÄ^G?ÒoÞ_FaŽ?òH›—ËŽ3?ææ¼Aå'·¿ç^-¢¥†ã¿é_ωþœ¿Ñéy«½ˆŒ¿Üœ\AŸ\§¿ãh4ë~AGNbll3FGL J2145.7+0717MS 2143.4+0704?ïö¦{ðL?P¡ø'÷¢?R³üiŸ?P¡ø'÷¢#?ï‰ýtÒíR?£"Àcè•a?€¢ËD«È?£"Àcè•`?ïâŸtÄQ?tz—Š—K?mó`‹;¯z?tz—Š—K?îÝòäMMä?ŠùçxåÐ?¢ Ñ»+!¼?ŠùçxåÐ4FGL J2146.4-1528?è·	'/`÷ÀFÑ|¯Ý©À:YyîÙgÀ<1£üÉêš@4I'n|à@Ì·ƒl?¿Î-_‰¨`?¿­0û›|?ø¥Èçdþ‡@ëɃl0«?ïó!3F¿ä½U¡E¿ëa¢ýpƒ¡¿é¡YìÛ`¿ëõ ޜØé¿ïÔ+{¯AGNfsrq3FGL J2146.7-1527PKS 2143-156?ïúÂò,ƒŒ?E<]*†S?Dô7MñÔ7?E<]*†8?ïüah¥VÉ?T(D¿-?<ôºÕIÃ"?T(D¿9?ï·eÌïX?€¦Z'Ý"Þ?'&ŒÄ9*&?€¦Z'Ý"á?ïëáPF‰?R©Tn¬Q?d¯¹võ8?R©Tn¬N4FGL J2146.5-1344¿ï}†µKAsÀFy—Ý÷wÀ8ë¼3øUÀ;‹Ûϟ$@Όïg+ˆ?÷ëŒ
dÝÐ?°y½!3+?Á±³ì{i@)4ÀÑìÇ@fûc
@…?ïGM1:Ç¿Ô[â¿Ó·'I%¿Ì¼&'j¿Ù"­‰'¿áœõ~DZ/AGNbll3FGL J2146.6-1344NVSS J214637-134359?ﵺ³bt ?«‹}²Ï?''S'b÷·?«‹}²Í?ïÄjSÏYÙ?£ Ç,>ˆ?}ÊÖS^?£ Ç,>ˆ?ïp9ì2EØ?f…qåN	?'øÂy·E?f…qåN	?ïTëB9¸y?ƒv*HH?•b—¸ÈðÏ?ƒv*HH4FGL J2146.8+0425¿ÏM"%"ntÀAµB€®IÀ:—Ù
LïÀ<3ycՒ@ò¤ø`@E"FK=ì?ÈèÁà_¦¯?Â4õ«?ò¸M¹Ç7@¶Å4ý㛿萘~'€p¿}è(a·Ä¿ê@õ~丿ëd&ñ'9¿Ç=Xlþ†¿ïÿÿÊPËAGNbcuMG1 J214653+0427?ïùŒæï?°?RØúrF#?IÌdCA‰?RØúrF?ïþi"ç?LCï'*Ö?/IfÁKB?LCï'*È?îñ	74ß5?–-?ub?? ïlŒ²¬?–-?ub>?ïú2_	ç£?>‡ãϧŸ½?G6ƒØaug?>‡ãϧŸ¹4FGL J2147.1+0931¿ï1Lª+À@×ÆûÒtÀ8h5qÑÔtÀ;Ò!¯}0­@'š¤†ˆ@u…zþ£ß?¡÷Hõ™L?¹"ö%j@t¥ß"9ç@h[J©q~¿Ï"ϝŒ˜T¿ãSßà›¿ç·|¯Ý©¿èØÍ÷o7Æ¿éd=ÔÌË¿èÈgÕÒ/AGNFSRQ3FGL J2147.2+0929PKS 2144+092?ïþnny€?"ÝS~DÑ?)gö6?"ÝS~D_?ïúÔÔé÷L?Y}øÉ4z?D¬¬X"ÎÚ?Y}øÉ4"?ï¡× $dË?†'ý˜{??‡Š7öæÍJ?†'ý˜{@?ïÿ"",?Âpät{?­žÿÚ|s?ÂpäsG4FGL J2147.3-7536¿²,õ®gÀBDR½<6À7™I¬|À;Œ›aöK@ÅeÑÄ®@íüºÑ!Æ?"~<*©?±>uf3'@;8 ؽœ@²\L=Ý¿¹¦'ác^¿ã‡>ùºì¿æ18‡0
Š¿æM= t¿ê‹P*º¿¿éWòeÊAGNFSRQ3FGL J2147.3-7536PKS 2142-75?ïð×`(?"ÓçZ`:¾?_ÚQ?÷¯¦?"ÓçZ`:¾?ïóò°?qOÑ?XçÛС×?qOÑ?ﷇ±
 
?ƒ¶Iªñ_?'¼—ý	?ƒ¶Iªñ\?ïÿ¾Kô>ö :œWøc?|í'êQ>ö :œWöæ4FGL J2148.0-0733¿ËãÛ…ªíÀE6€àe0À:S¡"I¦<À<j|>>ÿð@¤—»H?ý_ÂÞ6œ?Ä	Æ'l*¡?»JµA&!8?õ¶{ò¿¥@5˜þ")?ítM_.cÁ¿é§ ÉN=¿Ó +ïrC¿ÖH´å$‡t¿äú¬¤8Y
¿äÌqæÍAGNbllSDSS J214807.08-073347.0?ïûç¸f?7UÝúŸ?@cg¿£?7UÝú¡?ïüapŠŒ?XŸ÷=vÆ?<÷Ì{«N?XŸ÷=vÈ?ïïx¹·W±?j-¶P‹ç}?`‡FH¨O?j-¶P‹ç|?ïȒÓ8Áæ?dzÜÐ5l?{¶–cŸ
)?dzÜÐ5q4FGL J2148.6+0652?äûc°*V€ÀA™í|o½À9ñxKk8]À;ô÷Zï:@Q·&tU@BªA‡‰Í?²•>9x?ÎÃ핚0˜@jgÀ¹ï@
`ç\ðñÅ¿Ê-ªÞ•I¿åÖ]9–úƒ¿èºk5Øÿá¿ëƒï¾"OÙ¿ïÿúŒ—Ó?ÛÂð?˜œDAGNfsrq2FGL J2148.2+0659PKS 2145+06?ïíµ¶Ê€?dN,#?bJI5åá?dN,#?ïâz#.^?ŽdÿÊiù?m…ÜÑé¡?ŽdÿÊi÷?î4Ð~Êä?œŠ,êDL?¬²øQ·ù?œŠ,êDJ?ïÑ ‰Î+)?g
±Z­dÃ?w/»êl€?g
±Z­dÂ4FGL J2148.9-0121?áVÙ¦ˆ'ÀC£2œ4~À;Ïëe>HÀ<YLÓi©@Z$×$êp@ºñ-À?Àî^—ååM¿µ"ÄÐÿâN?öÃBZ£‹?úäd¬R?îŽñ"%¿äCHT,§ÿ¿ìlü›Ç¿Ü¨¡õ2Ç¿Ö5²~íÆ¿°Bœ ¡O	AGNbcuPKS 2146-01?ïó/È¢x
?Ub%³ºÙ)?Y n»ç°?Ub%³ºÙ ?ï·€:@?"»8чkÀ?'=ñoؗ?"»8чk¿?ïÉ\¥Mê¤?{uqûڗ?{Q­Y
®<?{uqûڙ?ï¯ñ/‰y?v®AÙÃ7?"´=¡Õ?v®AÙÃ94FGL J2149.1+6104¿ßÑתßy@mœBÁE°À9®cÂG7ÍÀ;{Š '§@©ù
G'@W¬Óª7?ávŽöS?Û	tBÈ@ò³Ù¶À@	ٗ
ô¿ÔÍÂ6Ƽ¿æÛz_A®÷¿ëáûbó¿ê(úãe¿ïb>ï)'¿ïŠ‹>‰AGNbcu4C +60.32?íµíÕtG?¼4ßjë?±êP'T]Ç?¼4ßjë?Úìó7…ª?Ô­±|g¶Ì?≆zd=+?Ô­±|g¶Ì?é%c&"Ô?°#Ÿ\þSÜ?Ëk'se°±?°#Ÿ\þSÛ?â¾³øYÃÜ?º‰¥Æ{Æk?ڂ˜LxF?º‰¥Æ{Æk4FGL J2149.6+0323¿äÙ:;þÉÀBNpCßÀ9Üëô°@¥À<F։äð°@ú‰*`¦´@êOyº×?¸N\Yr7*?«yQ'æ?ñS(ýOL@$xy8{¿¸tGz'î/¿çOš¿à±Šâ¾w¿áX¾]g¿èöTOãm"¿Ó[Þb¡_âAGNbll3FGL J2149.7+0323PKS B2147+031?ïùU²*ÁC?G¨ÅM‹±?J©7Tú÷µ?G¨ÅM‹«?ïþx´!ù.?D( ¨Æ@?(t½àmm?D( ¨ÆB?ïØoðôԒ?x)«
t@È?sÈ…•¶¡?x)«
t@Í?ïü»'ÒÎf?+¥{Ü`Ý?:#qiŒÄg?+¥{Ü`34FGL J2149.7+1917?ã͕ó´À:ZS2­À9ë—i=±;À<ó"Çz@4K¯«Ô°@·Zï9ß?½À©}è88?·Ù\Á殏?õ°
fóT@%÷5¿ç•žˈ¿ÜX'¿Ä¿çOÁ´?ã¿éxM·‡¿ãĀ˜@Ô¿ïþž
ÇAGNbcu3FGL J2149.6+1915TXS 2147+191?ïþà搷g?"HßVÃf
?!ñ–ô‰…5?"HßVÃf«?ïþGÿéχ?K+àÊ{˜?+€c'`?K+àÊ{™?ïÀ&O6g5?{¢
q· ^?ìØdÌe‹?{¢
q· j?ïþb:ÈP®?;
ºV¿
?)ÜSzõ=Y?;
ºV¿64FGL J2150.1-1410¿ïWõ$üÀFö5"_õÀ:¦‡¾¥ÃÀ<1£Œa¢²@ ×ÅiV?ù»À6âë?Áb@|që€?Â2‹˜z	Ü@€	ö#l@ՑíRÔ?îyˆLj;Þ¿çká©Ó¤¿µWXvb¿»^¾Š¥ò¿ãïî:ތ¿Ôéâéj'AGNbll3FGL J2150.2-1411TXS 2147-144?ïîÍ˪ Q?_Dâá7È?a24U_¯?_Dâá7¹?ïû²•?^å9©9-?C™7çõ³h?^å9©9-?{îL"ª?W£T?€™lÚÕe?W£V?ï¬	h•G?qa׭Ҏ%?"ý¥Ú¸î>?qa׭Ҏ$4FGL J2150.7-1750¿ÖaŽaK»^ÀG¼Û¾WïÀ:R}ü…!=À<ZS¸ä¸|@<pšœÎØ@2M	žs?¿Ã±ðþZc?ŸªžÆ÷m,?àv©ò´h@·FRʨ?ïî6>€nO¿ç8å#Û§[¿ç§¿Í
	n¿åà½D™¿äÍcˁs2¿ïÿÛb;ßTAGNbll3FGL J2150.5-1754MRSS 600-040574?ïú6œ½?Máµæ?G$é±ÔÎ?Máµæ?ïúóüȹî?[mèÊd÷?D0ÝKì?[mèÊdè?ïÎþ˜ÉD[?u©­ÃùÏÌ?x€³›]Ò°?u©­ÃùÏÀ?ïâë]…?]eg£¯x'?mû¢zéç?]eg£¯x4FGL J2150.7-2810¿Å±ƒ!3©rÀIâ`²È?À;^Ý÷—À<",·/¢@ 6üªàéº@%…EN¾ª?Ñrª?ÄÏi_?*¸?ôKà©"£™@ì&ØÜÐ{¿ïþÁ?|?ïþtå…*w¿ãàH	"
@¿Þ¯°ýcmŽ¿áøžö{¿àÖv~â^/AGNfsrqPMN J2150-2812?ïþ_ð°Ó¥?&+xjßÒº?*ôòřÜ?&+xjßÓG?ïþd–:?H»Ý§—xP?.ù¶œ^·ƒ?H»Ý§—xM?ïØ<_2C?yH)«Íq?sáüPfßH?yH)«Íh?ïö'n'*¹?EôMæß	?RtìÛªK?EôMæß4FGL J2150.8+1118?àõS37ûbÀ?»5*"8	À:å!ÁçãÀ<2\sž]@¸ˆd@H{Ã?ÎÁ".öŽ?¦cžœ?Õ=îãx	ý@ý]žk»e?íÜêâ6–j¿êåídòÈà¿ÙziÓe¿ßÀâ³¾Þοä´Ó˜A¿Ñ–éÜ'2ÊAGNbllNVSS J215051+111915?ïþ¸5D‹Û? |ÎϾsà?$|«·B@E? |ÎϾsU?ïþ]±¼oó?E±­ðÛ«?*$ä9Ï?E±­ð۝?ï÷|ðѺ?Wðs[¿;?Q]‹›?Wðs[¿)?ïó×~@ŠO?Aç"]ú³?XQ~ëby?Aç"]ú¡4FGL J2151.4+4156¿í•Ïd'%À"͒·þ¯À:_úŒ"¸'À<Ib(D€@ [ÿûù5?ù´ýö°Ì?ƙähŸÒ?ÕNŠø.%@«dÅ|vs@ø~©©1<¿é@¸Azsº¿æx6ÝâžÆ¿¸ÆÚVM?¿ÐäK3''¿áñBwô®¿è>ôÈAGNbll3FGL J2151.6+4154NVSS J215122+415632?ïg±/£Û?ýEœ®}"?žs	Ú"q?ýEœ®}"?ïî(ôŠU?{ªêZþth?a×ùu«'?{ªêZþtf?é[ž"í"ñ?³ý8¢?ʑ…¬I¬??³ý8¢?ïUO"8~é?:¸Ö?•V
˜ð"Ü?:¸Ö4FGL J2151.7-2749¿æ»ŸDTÀI-ž×ÆûÒÀ:ªDkiÛfÀ<0®û*®)@Ó/Â"'@[*'ñ¶'?ÖómàÙ??á4±¸tP@$è'4ù@
f´¯Êˆz¿àÃNžÉ"C¿å–Û¿
¡¿è¬R¾éµ;¿ê¢"FY¿ïÿþøþ"?ïòª¬çT8AGNfsrq3FGL J2151.6-2744PMN J2151-2742?ïûĹVŸB?K¨È"M!©?@í¥'ø¼?K¨È"M!¤?ïøyCb?lª6¼(÷(?OÒòuôÖ?lª6¼(÷*?îÊMTNÕt?–4?ô?£[*»¨¾?–4?ô?ïñ;@=‡s?T€òÕ%´?]‰"ñw?T€òÕ%¯4FGL J2151.8-3027¿Èý(WtþÀIb@îÙÀ89ÔñhŽÀ;¿?úÁҞ@æ°d@ýÙ<FØ,?¢T=nöWá?Ç°|ʀí%@è_^4h½@{Ã;~†C¿Ó¡ZX;*x¿æ‹a]¿ë¡}¾œ³¿ìàYq‹^¿íS›R×=i¿ïéjÇôö¸AGNfsrq3FGL J2151.8-3025PKS 2149-306?ï³#"Þ¥Ë?†Ï)ÜXdž?ƒ7ÈV?†Ï)ÜXd?ïê!rÖ¹z?ƒiU´T?eލ)F‡G?ƒiU´U?í"xld?¨g§êI͏?·ëd?üœà?¨g§êI͑?ïö¹Y$­l?EiX9™u?RM¶¥&t?EiX9™o4FGL J2152.0-1205?퐯÷'YÀF¹‰›õ"lÀ:Îÿ€¾À<k¹›— ›@ #Ýqµ¤è?þ%鞔«?Ñÿm]ü_?Ë!]•Ç?ýíG+7¼/?ÿ"IŽ¿ïýPÒ8r?ïÕ}«&‰Ø¿àÛá¨&$W¿Ûf®_ÏH}¿áP«>¡%¿ïÿä¡Õ¨>AGNbllRBS 1791?ïù¿Öú?H"{&-«?IФ›b?H"{&-ªù?ﵯ³×§_?—–5†F
Ç?'"
(~?—–5†F
È?ïuL!Â?ˆÂ›Nuc'?'OÖ{ǽJ?ˆÂ›NucŽ?4K±'?"Èþ¨ÒàÑ?¥ö¼»DæÐ?"Èþ¨ÒàÑ4FGL J2152.5+1737¿ÀçH,s+À;°¸{Üð0À;óiï‡ãÀ<aŒ¤¾Ê@zo÷ß @å^¼Mùˆ?͇4|´['?¢tâCñ5Q?ҝO0¿»l@ŠšrÝm.?é'Nž·Ì¿âZi7Ñþe¿æ]¾Anµ?¿ä$à¿ÈØL¿ãÎAvÂÔü¿îô›GðAGNbll3FGL J2152.4+1735S3 2150+17?ïûÍ2'?8¹ÆG[?@Ë7ƒ¯`í?8¹ÆG[?ïþc¶rct?CyÔÓT?)ĘÙÈ«i?CyÔÓL?ïåòñ²a?qÏw?j
=Mž
?qÏu?ïð0î˜DH?I6¥ÔW?_ž"Ïwnþ?I6¥Ôe4FGL J2153.1-0041?ìA6"xÀC߸ä¸{ÝÀ:é€æDmÀ<oèPïÝ@!æfRDpr?üÿüB?Äݦ¨ É?xCGŸÉ*ù?¶»]û)@txÍÇ?ïêLÚ¤%å¿ë^°ô)2¿œ›œNª³¿×«X¾ˆ…¿ÛoŽ˜´—L¿²WxÅ8¯AGNbll3FGL J2152.9-0045RBS 1792?ïÿ²$x@X>üÁ˜"õq?váïéêŒ>üÁ˜"ö«?ïþ)ŽSp£?E¨·—x6?-gÈõÇ4?E¨·—x2?ïú|?—+¾?V¡@Û
R?F£QJ?V¡@Û
I?ïü'Aø?1ñ{1Ì`Á??íð?Ü?1ñ{1Ì`ú4FGL J2153.8-1137?ì…?JœÀFÏËÉdcÀ9JÃÿž±1À<çq"Á@Øi¼\<A@7bR¯'?­'n®ßQ	?° ½ ñ
?ü'*߈'@›†é_¿Éó£»±q}¿åcn.±Ä3¿çBE¿é}þ."¿æà+²~m¿çÓ`žü/AGNfsrq3FGL J2154.0-1137PMN J2153-1136?ïþ³˜'t©?"Ýpk>?$Ævèµiù?"ÝpkL?ïýSöDR§?N]袡9?5`MÝjÈ?N]袡?ïÚØƀ?n*J¬A‹?r÷¼Àl?n*J¬A?ï÷	ÝäM?BBèé¤?QìD7çf3?BBèé—4FGL J2155.3+6602?ì>\Òx€Ö@"	¶o"5ÒÀ:êg¹MÀ;²ÎºÖ¨@Iß,ö®@p'ݽ¶?ÉÅ?º«3?ÈóÜ܉0@γ!*3@Ý:ÆF¡?Ë*é£OA¿ã7ÊaŽž¿êdkð"ò¿å¬"½ð¿î÷à†=¿ïÚÀ«VZ€AGNbcuNVSS J215520+660839?åÌöÝF'ø?ÊÊ/€IY?ÔfErú?ÊÊ/€IY?è㢼ϡ?ÍúSÌs?ÌqwÅÁ|?ÍúSÌs?êÖN5õ?·M'Ìc?Çô¦Çï(*?·M'Ìc?ëýý7=?¢·…L2¼?À#ãŒ?¢·…L2½4FGL J2156.0+1818?ìR%fŸEÀ;Èf^ê–À9æ7UãUÀ<-5Ã0l@!ŽsöœÕ?úP¿54•3?º‹ÉwWÐL?¸š¾²­¼¼@:g9Êüé@ù0´¨¾¦¿ê?ßÿY'í¿ÂI#ŸíE¾¿×yTŸêk™¿ÑBõ"ûƒ¿Þnê.£ˆ¿ÒÕ½aIñçAGNbll3FGL J2156.0+1818RX J2156.0+1818?ïøéÁfõ­?I^vÿŽå'?LXúd)L?I^vÿŽå¨?ïûçÉ£?Vá®
3"í?@càÛ¡s&?Vá®
3"ï?ï֛ˆ2Øê?wšåÖQ)?t²;擋G?wšåÖQ'?ï·4:úÊ?q;S(uó?'2ñAz
ƒ?q;S(uò4FGL J2156.0-6942?ãN¸ZH"ÀDH—žÖÜÀ:T}á­.¢À<((@éÈ@rK'ÎÉý@Eþw?ƺøcÿXæ?Ôûñ}†=œ@3öÂiœ|?úpH»ÊF?À *Aò闿ÌĈZ¬ôÀ¿êôZ5Ö|¿ïýA©î{s?®-ýê&$¿ïûpÿqºAGNrdgPKS 2153-69?î<ƒÒ"É{?¶ñ€¥nø?¬7ÂÖ³hI?¶ñ€¥nø?ìˆ?œG·‰~þ?¸‹ÏOòóÀ?œG·‰~ÿ?äËc‡¤ç?ºŸªÔ~
?Öi8ñÔ¶4?ºŸªÔ~	?놱æӖ³?´ùëC#q?Áå8d±¥1?´ùëC#q4FGL J2156.3-0036?ךQ›çFÀD+¿@OÂÀ9é Ï¨À<3ëGWL@+ót¡@ÜewS?µæD1?œöCW‡j?åB]"<@µýM?+¿è è½ïk¿Ø.}`ä¿æ'S‹'¿á' ¹Ée¿á~ˆÑË9O¿ê–ÿ5¿AGNfsrqPKS B2153-008?ïýÇÇé?,>íÁXtg?1Ç)ÇÈ®›?,>íÁXt?ïýÿZºüÝ?MÁÞD=?0*(€?MÁÞD=!?ïë±|u?i½	ûÚgŽ?dNƒ€ì‹†?i½	ûÚg¬?ïÿ…øŠ?˜ÙÂ~?Ý{>bÖ?˜ÙÂæ4FGL J2156.9-0854¿ÔµzÀF]xÀ:"¶ÂŸLaÀ<z™_·ö@œ¾¨Fۇ?üâqy¿ß?ÌÙäwä=,?ÌMbI†@ê̒@p"³¬¿ÜM[=…¿åÅý_çœ1¿Þd}§ö¿Ù)*›´üÌ¿àRh' Xпïù–m•/AGNbll3FGL J2156.9-0855NVSS J215650-085535?ïÔ	o>¤?uÖTŠr`?uûH`­¹»?uÖTŠrb?ïõ§}uÞ?oþàåÖQØ?T±Cöó?oþàåÖQÐ?ï³É,æa?—ՔtâR?Ÿ‰†Úc3¿?—ՔtâQ?ï™ÆÆr;"?t@Mûõó?‰ŽNcqÝ?t@Mûõñ4FGL J2157.5+3127¿ïñò"M¼À2="ôÆæÚÀ8I"ðÅÐYÀ;¬šÚâ9F@_t;@_‹Íþü?¡aÿÏX˜?Á|®¼Áfè@ c7ë(Øf@xhZ†­¿«Íÿý¦´_¿à‰¶b'<…¿ã'7oØÕð¿åU¥ïqó¿ìž–XœyH¿êÒxþn…oAGNfsrq3FGL J2157.5+3126B2 2155+31?ï´0uF
7?{ZPŸv?'óâ®}r ?{ZPŸv?ïáKÔß(?'|?ßß?n´+ð ØM?'|?ßá?íñ
¥€¹ª?Ÿ¢Dð÷=m?°w'Óú2¾?Ÿ¢Dð÷=m?ïû\ø	Ò?8Óä)õ¡3?BŒØ·®C?8Óä)õ¡<4FGL J2158.1-1501¿ïRT8 ‡îÀH<ÈóÀ9G+ý´Ì%À<"?ø="ß@'€ vÃ@¼w¯d?­@
‡‹ã?±"\éü@]Á@ŸS²¯•.¿ã™*GÒ'¿Ú²Í\¿ž'¿ãž¯çÜô¿äRÀí ¿âi%'×µ^¿å-c ŽUnAGNfsrq3FGL J2158.0-1501PKS 2155-152?ïý'+)¯ï?0'¨±õî=?3v¦²€¥?0'¨±õîz?ïû©K…5?Xˆ±1C—?AZÑéû-Ù?Xˆ±1C?ïØmI¾"?s&pcÁù?sÉ[y ¶v?s&pcÁó?ïì'`<y?T^G•3?c}ìŸÃˆ,?T^G•,4FGL J2158.8-3013?Ûõ26ƒ^GÀJ&k¤"ÉÀ6A7Cc,À:p¢¨6@Y'¹'m?üDÄö>¶?‡Ñ)ëЍ?¤ùÖp9£æ@tBÇû­@ñé…Àè¿¿âÈ6ºý¿Ö—¿¤Æ¿Ü´žØ»g¿ÙÝF'vú¿à;`ÿX±¿ÛՀºûiAGNbll3FGL J2158.8-3013PKS 2155-304?ïõ|9"I¸?X­=×b0?UŒ×lŽŽ?X­=×b0/?ï÷Œüâö?gôýí>Ü?Päæ:?gôýí>Ó?îÃöî2—?¢(ˆCè‰Â?£À'ŒÖ³?¢(ˆCè‰Á?ïþòœà?Cù±W)V? Þ¶?'î?Cù±W*;4FGL J2159.1-2840?Ç͍à'ÀJ<³åuÀ:ŽF@RÀ<AôÚ2@ C¼¹Ú+Û?û<\ŒÈп?ÁDœg)Z?ÄX¾Š@BíJ.!@vðéa­ð¿ïÿülò?ïÿÓ?,» ¿ßep½Wcê¿Ôo……t¿ã#-A+ÄT¿äK"=,®AGNbll3FGL J2159.2-2841LEDA 3218689?ïùÑÝF½3?F+|ÿG?H¸Šå58?F+|ÿE?ï÷ÜS1VÏ?hw—Õæ<)?PGYRcE?hw—Õæ<&?ï¾/½FÁ™?Ãgkÿæ?€t®O™«?Ãgkÿà?ï™K¹<ò?z­âӚt?‰ -°ÃŸ?z­âӚq4FGL J2159.8-4751¿êö÷€VñÀImÙ]ÔÇmÀ:zê÷Z?À<ƒdIU´g@t"aS×î@(?NÊhn?¼í™I'›?" ë!<¢?ÅËÀæå@¿Q$_Û³?ãÁ­Ÿ`¿ãà%¿­)™¿æ9Áø]tO¿é+f ïÀ¿ïýŠoZ*ï?ïßM œÃAGNbcuPMN J2200-4751?ïÿ_à`MÞ?Á­fBÚ?óöDK7?Á­fBÚ?ïþ©³™#?@»q+Rdé?%dÆmÎ_?@»q+Re	?ïë"
‡µV?eA«™A#?dkõxJ«h?eA«™A'?ïÿ¶"A0 >ú…!0cµ?^ï³ØuH>ú…!0cƒ4FGL J2200.1+2138¿î±BUpÍ°À:>$þ½
À:-m÷T`À<KvY"±@.WÁ²èJ?ÿ¡mµ?¼×Õ˜8F?°R,—Õõ?ô'p*4†ð@)ˆh™Çg?¾†ýOüm¿Ý-£ùnì¿åœº¶IӉ¿Óú D¯¿áƒsR3Ñ¿ëwÁ½¥AGNbll3FGL J2200.2+2139TXS 2157+213?ïþòƒ$ƒ˜?³vH…¯W? ×ͷƆ=?³vH…¯M?ïþ&õ‹¯¼?H'6pÉË?-§EJ¨?H'6pÉÌ?ïôt¢Nö,?dˆ)Ú ?W»b©?dˆ)Úª?ïýƒÈéÞ?$h8Ú(+?3ḷ‰½?$h8Ú(34FGL J2200.3+1029?ï—ÇñCNÀA.@…+NÀ:x3|.NÈÀ<PX(¶¯@¶Z
'º@ISù|X@?Áñ"ÂÅ7?ž¾}‡Gåû?Ú¨Ë%WÓQ@I$ß]s#?ïÿûB«÷¿äÜ)áû³¿ê²îO'¿×ôè_Op׿éL÷?7á¿ïÿ¬)ÜrAGNbll3FGL J2159.8+1025TXS 2157+102?ïõLÃmŒá?[åçÿÆ·î?Ufy$æ?Ý?[åçÿÆ·â?ïњÆ`?‰ÛfÀd?w2œÏòz?‰ÛfÀd?ïZÆpžUÛ?‹AlÐÚ?"§1ì5D¸?‹AlÐÛ?ïŸÊÂñdE?tëd5¸?ˆ
OC¦î±?tëd5¸4FGL J2200.7-2414¿äÅP4"·_ÀIÎWâ?$ÙÀ:•'Àa"À<'F…@J'KÇ~¯@e9Z"¡?Áþ{
ã3?©¤2|]?æá¤_Æ95@
Ô‡Spë¿çtî>Œ'°¿Öµt@™£*¿æu9½æÕâ¿Ùè<œh¿æ'Z«GA¿ä)~HÛ;%AGNbcu3FGL J2200.9-2412NVSS J220036-241428?ïþîMÆZÜ?t†Y¢h?!#šR9?t†Y¢h*?ïþ0?<S'—KŽ'?!"þ|r?<S'—KŽÖ?ïó´¦U­¥?cTH7Ff™?X–³T¤¶Ü?cTH7Ffž?ïþOuå‹&?Qg"§[?+¡§M¦5?Qg"§Z4FGL J2201.0-5907?îâ‡hqÀGW}|,¡IÀ;:p>V}À<ñ8Ë@ ¥xJŸ?ýs¸ÿnx?Ô—ç—S?Üþ#[ú§¦@gGzÕ@:ԈØ׿ëU ÃÄæN?í®ðBóš—?}Ö¨¿âGò½¢7x¿éØb,E¿ºRÅʤÿAGNbcuSUMSS J220107-590639?ï ä°CÓ?žTQÝ	?›ãi÷ª?žTQÝ	?ïޚ9…ÏÌ?Ž¹=ˆR?p²ã=?Ž¹=ˆR?ìü¬à!•?¥œÒJK?»˜þóP?¥œÒJK?î£:)–®?˜Ôq+"N?¥Ì_íf•?˜Ôq+"P4FGL J2201.5-8339?ïä'ÿqÀ?¶,ºs-õÀ8¨á¼©iÀ;j¥P‡@ž«"‡@î.|M•?¨ß T« ?Âü]CÆS@ï»@ãÑ C—Y?ïGòrxÃ`¿å&H.ÿæ]8TÛ#¨¿ç÷#b…±/¿ëãIEÄ/o¿ïþâ=ø3-AGNfsrq3FGL J2202.4-8339PKS 2155-83?ïõ+ބѬ?T)~zBy?U¨Bö\ª6?T)~zBr?ïõP=½·"?f÷Ρ2RZ?U_""×Z?f÷Ρ2RZ?î~x4Mk"?´ýÏÄé?¨|»)Mä?´ýÏÄé?ïåâÁüÆÐ?YgtSAÙ?j>90?YgtSAØü4FGL J2201.5+2950¿ìۀ¸+¯þÀ4ë9Ÿ]ÿÀ;×gZ'À<ˆ~aßï@@)iÛ»Ó@^ø³Û?Ï7‰I`œ?¶¼¬™%«`?ç¬ÄÉ$¢@k—ˆrTÜ?ӇŒü¨1¸?ïë뫵%¿æ⤥fVv¿×–£EG¿êaQžÙ•?¤,٧ѕ´AGNbcuRX J2201.3+2949?ïîv🿤?_þlI•M?a‰`@\Ï?_þlI•S?ïúO^.ZÈ?eÌ*"}?F‡F"áÄ?eÌ*"}?µ…m‰?"4§÷s|?‡'ž¤ž?"4§÷s|?ï¾ÍËÇ~?ntJ/ñÇ?€L:Ž v?ntJ/ñÉ4FGL J2201.8+5048¿îᢃÃèZÀdg`ai§À7²š²žM^À;L(Ê#¥!@¶Ý®òFY@€_†xT¥?›öAô?Â4J@Qü£T-@ ·áXJ¿Ôy!Ôæø¿ãyk@Àºp¿èÊ÷uR¿éñ‹@;¿ì¥2Ÿ9–¥¿ïÿ»!(ĚAGNfsrq3FGL J2201.7+5047NRAO 676?ïòÙ׀æ ?]×u<¼wû?ZLPþ3Â?]×u<¼wú?ï³°ñäi°?®§‡$À??ƒÆå"=?®§‡$À=?º•VA?›@¥Øÿ€Í?¤GdVª›í?›@¥Øÿ€Ì?ïýÁòáé?(~þUs?1ðhð·+÷?(~þU4FGL J2201.9-1706?êð§5ZÀHØ#|ÜÊqÀ;Í¥,tÓÀ<Òï ´«n@$/ÿ¨Â+‰?ö…6+‡?à«úYÍÑ°?–´3<²&È?¬ÊÎþÙº?þ¶ìM›"F?çøäb•¡g?ÝYŽÏ[¿å>^‡tÔ¿ïÿZS2¬û?ïþSW•é¿Îîì\_&AGNbllRBS 1813?ïÿz£dQÝ?ªÿ@D?«"uÄrk?ªÿ@x?ïýñ`RÊ?`mA¹4«}?70týi¢}?`mA¹4«}?ïÀñå{0?—O~Z@µ?œáÃPš?—O~Z@´?ïüTc`†?CKY$\‹¦?=\ç\ûÊÆ?CKY$\‹v4FGL J2202.7+4216¿³r°³/,À$ãb¥ç…¶À61â§)¥À:¤Nér@¸¨§ÿc@%@FA,ñ?"•1f:­·?®Õ¬€?T@$YH¾H¦@ UšSÓ¼«¿Ä¿('!-¿ÞýÀà…f\¿ãӉX=¿âÐíޕL-¿æ;a3v¥¿å(ê¥$èAGNBLL3FGL J2202.7+4217BL Lac?ïЖˆÁ©?y†2ÎOÒ(?w´ý;Ÿ,"?y†2ÎOÒ)?ïÂÌÕ,?'ùmV'´?~™•}éþû?'ùmV'µ?ï{h'ò©?èpÄà$a?'û!ªÁ?èpÄà$a?ïétyýF?`‹˜"LÐ?f዆¹¹?`‹˜"LÑ4FGL J2202.7-5637¿î'ÃHsâ;ÀHÓþuóÀ;WçS`Ð$À<ג:)Çz@ —½çו(?üì*EMçê?˯ >#|?²t\É.²›?è|îh(?ûÊòìq-?Ú¡Ü>ñ§?îÌ Ÿ²¸O¿âsÞ-è¿Ï¤Váä-¿ïÿò~#¿?ïÿ·ÀÌ
ŠAGNbllMS 2159.5-5649?ïýM¢Gå?7WkÅxTZ?5'ë•ÀÓ?7WkÅxTr?ïÕ]‡ÎúÆ?"}ÉÌêV?uQ<'œÙ?"}ÉÌêW?ï|y'Ià?ŠfÅJaÙ?pϼÃû?ŠfÅJaÙ?ïw1­s«?†!'‰*q0?'ùÊQŠ­?†!'‰*q24FGL J2203.4+1725?ltÃÀ=£µ¿j
»À8:²ái<À;§I׺f™@•äô¶Ë¯@ÚŸb0w?œý( Ëß?³"a†q@ö_½Õ¹@ebÉ"ô!¿¾¡O›s¹`¿ß:ÆF¡¿åK~îóhB¿å7_ÞO¿æ¡!þ'|r¿érR,ó~AGNfsrq3FGL J2203.4+1725PKS 2201+171?ïÿ%Mbþ?¾—™§g¾?ÛVS 7D?¾—™§gé?ïûîÀ^(?XvÒù—;[?@Dÿš‡e…?XvÒù—;T?ïäþçž«?pO†Ñ³µ?kaãUN?pO†Ñ³°?ïÿÌßöU]>ð-ÅTÑ¿S>ùÕQIÌ>ð-ÅTÑÀœ4FGL J2203.6+6751?ш8UuMA@#ç@š$À:[¤ˆ
%À;ÚVų-@å‹
µ'@—Ö›'§æ?Ï"¸ß/%?Ç¥ÚZ)O?ù Äeõþ@5àŽ5?íõ«gᑿèÿ|'1ž¿èсèM¿é¾x`¹Ô"¿ïö¡÷6-¿êÐØËЯAGNbcuLQAC 330+067?íþiäڎ?µ†4ûÛ°ø?°"°Ù+‰?µ†4ûÛ°ø?çû'?³–?Ï3âC9?Ð	ݱ€˜Õ?Ï3âC9'?éC€%´¢P?¶·[»¾n?Êñÿi-v¾?¶·[»¾n?é5«ùq?©¦É÷+(?Ë+²P>?©¦É÷+(4FGL J2204.3+0438¿Ñ°ÃáÀl9ÀCT!BoçÀ:
,·îïÀ<Qé{Y<²@ÖIGF»{@­|ÀDÿ?»"žñ-?¿ÆÕfú5?þ`Î\‹@Íêæßó¿ãӕ:a%¿âôÇÝÏ©v¿ãiÇåv¿çôÓ˜A¿æZ1¿•¬¥¿ænnD—àAGNbll3FGL J2204.4+04394C +04.77?ïôPüFØ?VSg¼@{æ?W_îrNÔ?VSg¼@{õ?ïúâá°?_ù
üâÄc?Dwðy?¾`?_ù
üâÄo?ï˝Ï/"(?{t^aŸˆ?z1h5ìÎ?{t^aŸ†?ïÎü¬¬ÒC?dy"qì
"?x©©–Ýø?dy"qì
4FGL J2204.5+3634?Í9\ÇPÙÀ.\ÌîZ¼À; È1\™^À<J'Œ"Þ!@ <7"À@§äRµ?ÅÑY¹Ú¬´¿£§àYF˜?â"Jb#á‡@+
s†	š¿ç|'ݽµÙ?ï·õÿËþ¿èÉ[]ô§Ý¿ås]û]Ùпãõ
}ìêÏ¿œkÊÃ!?AGNbllMG3 J220423+3632?ïøñ4Óù?Kçì#X%¡?L;,°Я?Kçì#X%?ïý̸5Nô?Jéµoö"Ë?1š>Uˆi?Jéµoö"Ê?ïÃÞÆøã—?~¼m@±å?~œƒŽ4‰?~¼m@±é?ïî?T­ÅŽžµ?açóoìæ£?T­ÅŽž¶4FGL J2205.0+7432?çî0_@£@.dvò¥¤jÀ:å*Óa,À<ap9N@xs²Ì›@ùš‹1!?ßš"Ñ
Ÿ?è…ë1;â.@l Ÿ²¸O@¢ÊšÃe¿ï}Ë<©Ôz?ïÿ÷œ"/¥¿ÎI‡9£¿é1ÿŒ<¹Å¿ìËÃAe%?܂›üu¼AGNbcuS5 2205+74?íÃ.øË{ý?½•lE]#?±æˆ9¤ ?½•lE]#?ç0¦m­"Ý?Óhó!Ԝ?ў³$¤ØF?Óhó!Ԝ?êL²xøwî?«N'S9ù?ÆÍ6 D?«N'S9ø?ãÓd†RV‰?ÀÀU˜a(À?ØY6ó[Rî?ÀÀU˜a(À4FGL J2206.8-0032¿ïH3®EV|ÀE4Áü28À9Lå".(1À<ºß%•@r=Ô¡ØW@?› 'W?±g¨A
wž?³¯—‡Æˆe@šfH3u@c,°ã?ßüÒ¹u×ó¿ÜÛëc:âÕ¿äa~õÿK¿àA¨a2Ÿå¿í'C¿rq7?·ð©Jç…AGNbll3FGL J2206.9-0031PMN J2206-0031?ïûÍGž
?8ÿÀTÿ?@Ëúá‡Ø›?8ÿÀTÿ*?ïýV¤[t?IL÷2U1Á?5JÝ'äZ6?IL÷2U1Á?ïH‡•"?'Gâõ$á?–ÿ/-Mv?'Gâõ$á?ïü—µ·ä?0A"ÂÝ:Z?;G2R@á®?0A"ÂÝ:?4FGL J2207.0+3607?¸+Þá7À/°ÿŸ‡ðÀ;i£ÙŽÀ<c…Ò<xV@ 3
ž¤@IsÙìp?ɪ+¢› ?ž(Û@'üõ?Ö¡sÕB<@úm‡	¿ï¨P!ӏ?ëU°€æÅF¿â`‰ãC0׿éò"ý[
¿´t×~'¾D¿è '+"ØAGNbcu1RXS J220708.5+360935?ïøÙ݀š?M&ˆ¿÷ÎM?O˜˜‰ý'~?M&ˆ¿÷Î<?ïþŠµ&úš?E6¬(ˆA…?'T­Vg"?E6¬(ˆA•?ï¹r3?€ò@ý®¹J?£ûó?€ò@ý®¹D?ïõNÒ[ºP?K©aÄ{òK?Ub[H‹],?K©aÄ{òS4FGL J2207.1+4316?펙• àðÀ$FÎô©‹À:"qDúÀ<	Ÿ)üRÌ@ ¡™Ê–çŽ?ûèQÃA2Ð?ǯI™§"?ÐÐÉ<qu@v.	þ†ƒ@	n(Ãm¨¿ï²¾™-c?ç'!þW‰T¿áeHŽå
±¿Ù¤þývŽ¿Ó-eÿ8Yä¿ïÿäë8AGNbcu87GB 220504.7+430144?ïñqŒD?û?[ŒÎ\ºfÐ?]çw€?[ŒÎ\ºfÕ?ï÷"x‡øý?l:Z¡¤€¿?PÙðâ?l:Z¡¤€Á?í{]a1?¤BU;"˜Q?´%÷'N€?¤BU;"˜R?ïÂðâ5WS?oÃ$â¯À
?~‡ŽåTV;?oÃ$â¯À4FGL J2207.5-5346?éêÆv"ÀHóþ®û+À9yÝ÷vÅÀ<j'¨
У@oPk'kT@P.Ë?«¢•Ûc?žù
¦z ?íã™BÞç@§¶š0m[¿Ú˜Ïö¿â[ýÂ8T¿æ¼ìOIo¿å—,×Ï_¿êú³fÊ9¿ÎƘ*XÄAGNfsrq3FGL J2207.8-5345PKS 2204-54?ïþ'ö.õ?%¿(H±Ž~?-Æó?%¿(H±Ž?ïþB•zÞz?J¥êd/ö?+Ö¨RL†?J¥êd/ö%?ïçdåzãÚ?lô"(Š2?h›…$Ñ?lô"(Š'?ïÿ'gîT?ç=·+?5|kß?ç=¶"4FGL J2207.6+0053?ÕŽ]×GüÀD×ú~¶¿DÀ:±Öv™ºQÀ<Uq€Ø@æ«͏À@ÂCÜ΢?ÄàĦbªÅ?¢ñ·¤ã–?ÝeêÕÌP@â«¡.
"?ïîÎ_¢¿ç0Èè#¿æfA¬Ž¿ê}ÅB"пÊX‰m~¿ïÿwD;ÏAGNbcuPMN J2207+0052?ïÿ23™ý?õvjsD?½ùŒÀŒê?õvjsCé?ïþ†).šÚ?C²ÙÜBú?'mRYð?C²ÙÜBú?ïè *ƒeZ?gàq@У?gßÕ|š§[?gàq@К?ïýXàJu?)üýÄP?5?(ý¬K;?)üýÄý4FGL J2208.1-4507?ߒ'+ˆ²§ÀJ|ÁÁÖυÀ;É7PÏ%mÀ<òrâu«~@!ï0ì\?ü"þ_
?ßÓp?ƒ"µ?ªW[AÖJ`?ù²v‡›À:¿ïÿæ4|ßO?ïüv¨ÓÉ@¿ÐeºD	Y¿Ú::c~)§¿Ü˜bŒè¿ïïM•µ‹AGNbcuPMN J2208-4509?ïÿT€Ào?…Ù̙ª?oÿGò(?…Ù̚P?ï÷Ò[ð$?i—¹´e¤¸?P[ÉH¸•?i—¹´e¤µ?ïœ@`ÕE?Ž§ýâÅé?ˆïÿgÊ®š?Ž§ýâÅé?ïä¿Å1Ûp?]®Z¯Ì?k@:Î$é?]®Z¯×4FGL J2208.2+0350¿Óˆ–%"±ÙÀCõº² À;RӘ˜èšÀ<«ÏèàÿŠ@oŠD¼óf@ᇿ}?Ìb~dßӐ?¿¶œ´¬?òÞU‹Lϼ?í¥ð¼¸yü¿îÛ
F9 ?ïã>"¹…È¿à"ä0– Á¿ä!Fkõ ¿áz+ª¨µ–¿ïÿCaԆUAGNbllSDSS J220812.70+035304.6?ïÙëuw>
?¬ì)­`ç?s
ED`û¥?¬ì)­`ç?îÇiNCq?´Æé@3kX?£‰kûÉ?´Æé@3kX?ï~@WÏ ?ˆŸ,³lK?7õÎ?ˆŸ,³lF?êlë(ᩇ?®#L¹5ˆ?ÆLS\yYà?®#L¹5ˆ4FGL J2209.4+4329?ïêu¿ À$h'­ÄÉÉÀ9ºÆîj¬À;›Wëy`>@˜%ä@|dý°šg?·¶ böð¿¨*£dÄ?ñ`ú@jµ§l@?än.¡©¡¿ènÓr'¿åHNöÞ¿é¼ÿ¿ã¡Ö^ÆßοÚÒÁÃÚ4êAGNbcuB3 2207+432?ïûДB	æ?=@R.Fñé?@½®÷Øg]?=@R.Fò"?ïül7IA?Q'UÃÖ9?<›EµòÙ?Q'UÃÖ>?ï¿m¶ã‰?{†	»Á¸Þ?€$¿ÒGÅ?{†	»Á¸Õ?ïÎV‡'º?e6ÁvÀ¥?xÔ¼7w¢Î?e6ÁvÀª4FGL J2209.7-0451?ã뵊yë‰ÀFÅ£~õ©À:aµÁŒäÀ<JO¾"4®@ âóÀ×v?þD¸)§™?·V3M÷ž¿¤"4áÅ=ž?îRàw¤|@ÕºåÈú¿ì¯©Ggž¿Ø†d¾E s¿ÏöN»ÏÏa¿çȧ¤WÚ¿Ô³çƒ?´æÐÙ÷­¡AGNbll3FGL J2209.8-0450NVSS J220941-045111?ïùbÛ_I?F¹êšÙÉú?I¾t''Ú(?F¹êšÙÉð?ïü$ñ?SéwùÊâ²?;‡Øwu€?SéwùÊâ¶?寧!õÛ¥?"ŸL]*y?†Uw'‰"?"ŸL]*{?ïê,µ*#?Z"UÈ^Ï?eÓJÕÜõ½?Z"UÈ^Â4FGL J2209.8-5028?Ý,›úڟÓÀIƘÀ¤ À;Lï͂Õ2À<¤u‰ïØk@ÖÙyÙ_Ø@œ÷S½?ÐÉý·{W?±äØfÌh?ã´£
[£•@Úºch°?í«ñŠò6ê¿álÓu]¿æÂIá nu¿ßmA£¹X¿ë®Íb¿ï÷9R1%<AGNbcuPMN J2210-5030?ïþ¥Á÷Û[?"{Ã4&ì"?%£à'J]¨?"{Ã4&ìd?ïþcjsX'?E—¿ŽS'"?)ÉXÊwäÀ?E—¿ŽS'?ïääÀ÷:Þ?sEí¿Ï?k?Å!7?sEí¿Ó?ïú»¼¿üD?5
~u²íü?E
ë{?5
~u²íä4FGL J2210.8+3203?ì'p ÜŸÈÀ3Í_™Ã‹À;ÜjžÚK;À<ߧ[#<E@$œ^o÷à?÷&ª>,‹y?ѾÇüX€ ?ÂZ<¡ñ×É?ñÑU¡Îò@"ì3D{¿ïÿÿÊPË?æ´yï°&¤¿µ"¦:'ÌF?ïþŒÝôgp¿âüvÄ¿Ìp÷äÓ~ÃAGNbcu1RXS J221058.3+320327?ïþŒXW5?+ßG'Ý
ë?.W:zŒ¾I?+ßG'Ý?ïúdhêÛÎ?hÑÚª"ç¡?Fn\TÁ?hÑÚª"çž?ïã"Ÿ!õD?révb›¹?lÝ`Þ
¼©?révb›¼?ïïZ §ÏÞ?^åØ/±2£?`¥ßX0"ª?^åØ/±2"4FGL J2211.0-0003?¤üßp%ÈKÀEy¥q"À:ÆîᵒÀ<tÌežÀ@ ZS6Ñù?ýP"{rg&?ÊXyÿ…V?»?äq"&Á?óÂíÖ1Ð]@Òì؅è?ïÕ1U¡Ï¿æŸÿ®—¿Ý‰9"ÛòZ¿ã^M"0ÉÌ¿ÂaÉɍ'E¿ç]Ä×5AGNbllRX J2211.1-0003?ïýš­xoy?0Ƙ‹ü?3*"<"0
?0Ƙ‹ü?ïý.tì¢ë?P²=ÝÅWÍ?6ŒXšè¤|?P²=ÝÅWÚ?ïça²*$?qI¤á"'E?hžMÕÛøE?qI¤á"'??ïÙÛ7?b‰DÇÐ?sd7¦D?b‰DÇÐ4FGL J2211.2-1325?⟝1¡—ƒÀIÌ>1"÷À:ŽŸj"óÀ<U¢šÊB@§"å¡ì@™f`‡)U?ºöÄBÃ<?¨æª"xu?ßÁ6+57ð@Ó1p:z¥¿ÄnÖ·Ý&Œ¿ã[	pÂ	û¿ê֛'§å¿ç‰âÂW}ë¿ïÿåþÌú?ïÿ}Ž¡AGNbcuPKS 2208-137?ïÿJ®;¼?ëéë<7Ñ?ª8ˆ}QÀ?ëéë<8­?ïýù}Ⱊ?H@>ȕsU?04ê{/Ô?H@>ȕsa?ïâf:€?kþ,Ââ÷Ù?mô™Åò\?kþ,Ââ÷Ü?ïþè	Öo?ëÈx3kD?!b™Ýç?ëÈx3jÓ4FGL J2211.4-7040?Ú\®jynÀD~	VÀÖõÀ:÷Óc¿ÂùÀ<À!ˆæÃï@Šˆ¯'@¢P¨­?½¬/ô9xG¿¨•Ú¦‰¨?ìUÐììýÅ?þ•'¦8
Ž¿àr·B!À¿à-YÕ^kƿ剀Fâ<¡¿ã¿ÕØå	¿à­á¥!¿Û¡œ1úNAGNbll3FGL J2212.3-7039PMN J2211-7039?ïôºÒ»?Oõ<!ñ…£?VŠZ‰Íô˜?Oõ<!ñ…'?ïïâÉ35?t׃)T{Ö?`6ýÌËY?t׃)T{Õ?ïÞE>¼ó
?r½ÌHŽÃ?pÝ`¡†y	?r½ÌHŽÐ?ï҈Ñ,#m?bص "Ä?v»—iîI‰?bص "Æ4FGL J2212.0+2356?ëçÄAiÀ:q£±JÀ96ÁU FÀ;㶇*@´¸­@óŠ§ß­?¬ç…›ñô¶?¸É»{Eq@Á _ò@Ó/m¬¿Åº™™n¦|¿Ý7zU0³ý¿âÉUÐ-¿ä×àŠ"(¿æQßp¾Y¿à—àýy½AGNfsrq3FGL J2212.0+2355PKS 2209+236?î£s‹,Ïû? €0‡³gs?¥ÈÇM3B? €0‡³gs?äèÈÑÍÈW?Òp3gËÅ?Ö.n\doQ?Òp3gËÅ?ë^‡Œ"Þl?©Üøk8S‡?…áÍì†N?©Üøk8Sˆ?ç$[T҄[?±ÊÚ±Í'4?Ñ·IVZ÷J?±ÊÚ±Í'44FGL J2212.2-7251¿ïgŽðžcÀCËØà†8À:ùÊd<À{À<"+¯±3@ˆºÏa@¦T…"RX?Ðkcü(Úë?¶å¸åº/?é¢Nt@fãr«™ ¿çò/ýô¿æ\°ožôL¿ä–_'‹¿ç!·à¬~¿ìì¿B ¿ïÿA(¿;ëAGNbcuPMN J2211-7249?ïýÀSä\?0"<¥Ç?1ÿ`Ý"?0"<¥Ñ?ïùœw—¸¬?eR›ÇøÓ?IŽ!¡KÈ?eR›ÇøÐ?ï½he§ï?€ŒíEŒÌ?€¿eæ–9?€ŒíEŒË?ïè`ð.÷?Xy¡Ûy?gŸÑò(?Xy¡ۇ4FGL J2212.6+2800¿î*0•¤zjÀ6ülü'œþÀ9ëÕYcH¥À<O'h˜p@™õ *­S@ãøÀpø?¶t·7_?³ÛÙÚý<+?üüYÒÚ-@X±G
V?ïäC '?à¡
+a­š¿áÑ0ߛÜj¿ã•"ÁËçÊ¿ßÛڜCB¿ådÏÝùDûAGNbll3FGL J2212.6+2801MG3 J221240+2759?´´¸Û?ƒ¤ÿÌÃf?‡ÒÒÑÈâ?ƒ¤ÿÌÃg?ïÓ°…ò¨?ˆz?v'¹=¬K?ˆz?ï2çÔ@Û?'ò^öl?™£}×äj?'ò^öl?îYجž4?—M™–tN]?®*bu6Ç?—M™–tN[4FGL J2212.8+0647?êõtdºúÀCfƒ#5.À9ÒÏr™zÀ;Ø£'@ßÄ@/1ÜF‡@m«w?¾fLæ¹Í?Ãx~‹ì@'pŽ@ÕO¨3æ?Ӝ=bá÷¿âS	AÈ!l¿ãܸ2¿êÊ©ÂÉn¿éö•žoû¿ïþ-͘¤§AGNfsrq1FGL J2212.9+0654TXS 2210+065?ﻇ³g%b?€÷Œ qº?&6§Í?€÷Œ qº?ï׸ÅÄ2?‡ú¸ &@Ó?t#æò³?‡ú¸ &@Ñ?îØ4ÀíR¯?– ÔåŽL?¢|³ñ*Õ?– ÔåŽO?îùã¦pro?†ÙŠ¿®? aŘøÙ?†ÙŠ¿®4FGL J2212.9-2526?˖[î…~ÀÀKHßÞøH|À9Æ÷ê‡È·À<f1ØÀ @©þÁ'…@DAãÐ'?µ_ý–™4?ÀT5¡Íoµ@áDS@fý5uWÆ?ïeç}R;¿Èô 8Y¸®¿äövŸ´'¿âŸb2Ô¿éKòJ·¿ïÿõž}.)AGNfsrq3FGL J2213.1-2532PKS 2210-25?ïø6´CÈ2?NnWstL?O%.ðß:E?NnWst6?ïþ¤Û
B?DÔSVl9?.Õ²O+מ?DÔSVl<?ïPïƾ)ˆ?YåRhQ?•â(:Îå?YåRhP?ï÷u¤ôQ?B2\:«…í?Qñ¶[î?B2\:«…õ4FGL J2213.5-4754¿é•:eÀJƒ2a|ÚÀ;†¯²	ÓÀ<²§$œ—{@ ´-"¯¹?úèleƒè?Ð04:Å"ß?ÂîräÎ÷?ò"ÏÝù@'óƒðºé?ïû‹'™¿ìYÙ$Éã俵Ûc¾k`¿âc€4
¿ÃÇT}ZÉ¥¿æí¦a(9AGNbll3FGL J2213.6-4755SUMSS J221330-475426?ïþôæØ? "Œ™:Ø ? ¿ñŸÂpl? "Œ™:Øm?ïýï˳ž(?JåcJXƒ?0¢c»ñ?JåcJX~?ïèFCÖD"?n¢~§>Á?g¹¼)»Ý¦?n¢~§>Â?ï÷a…°öï?CÑ>ú£íË?Q<ôž #?CÑ>ú£í©4FGL J2213.9+5948c¿é¸a\Bv@½ZiÀ:ôÏJVÀ;N[`xæœ@É"
–ÜÑ@l¥³Û?еHŸ¸?ÀNL(Í~£?ö'SZ(@GMƒA?í#Ýàpm¦¿æ͕ŸŽü¿éÕÀ˜áä¿å|ßÿÚkF¿ä9AG`¿ïùÅôkwGAGNbcu1FGL J2214.5+5949TXS 2212+5958?ï ¬Z¯?ŒÌ¡OÖñÕ?‡Ôé{œ–?ŒÌ¡OÖñÓ?í@çaŠ3?Æ.JrԂî?µøÄó®g·?Æ.JrԂí?í²µ€a÷?§&pzÓÀœ?²jSüðM?§&pzÓÀ?±ßE?"Mõ,UTŽ?¦ÎTâ¹?"Mõ,UT4FGL J2215.4+0544?á×~4™ß£ÀCý—€º¥ƒÀ:¯¬kbOÀ<ióB'[@^´¸ƒê†@†ƒd£î‡?Ärj@:­¦?´Eyܺր?ðé›9¬Éø@ár¤P¿ï«.ýn€;?ïÌÄ¿77û¿èê~eᆿԑMjÙ¿çÂ[úҙ•¿ÈNÕ:¯~]AGNbcuNVSS J221513+054454?ïôo4*?WvD‹6Ï?Vá!—«Ë¨?WvD‹6Ê?ïö5$>å¤?eÊîYlût?S•·'4¸?eÊîYlût?ïÒÛÏýƒ—?w…ÕBž£?v'>3ô?w…ÕBžž?ï´5¶»ã?stC؃žì?'ò¹Q¿?stC؃žð4FGL J2215.4+6105¿®7Ðfˆ³@
ª:›À9æ†t"çŒÀ;edù~Ü@GK1¬ ]@øÍ ¯¢ð?ÌèæˆàŽÌ?Îü¿¿s@Õd¶býü@y-Å
5¹?îFÉ))?šg8ÚxBB¿çÄô'6ô‰¿æºÊ×)G!¿ï'>ˆPò¿ïíx:¤AAGNbcuNVSS J221507+610506?¾Ì'ö?ºçg‹ÿt?ì&m½¡>?ºçg‹ÿt?ÌÁñ±°Ê?ʔžV]ˆ?èσ""øM?ʔžV]ˆ?Ônúü?¸Pëü¨JÕ?åýȂ¿ü?¸Pëü¨JÕ?Ð,êV°¯­?¬Í|í:ä?çéŠÔ§¨*?¬Í|í:ä4FGL J2216.8+3103?ïûw%MhÀ5Cú*ÓéÀ:'S"¾À<6­•Ïà~@êûRò\@¼¾´ .?Ê\#—^ÖÐ?Ìvh&¯í?þrÉä»@ÅR¥>hq¿­QƒD1w
¿Ùè:œ3&ô¿èï^&üĿ拃ŒÚ¿ïýŒÙT›¿ðAGNfsrqS3 2214+30?ïBžÜÒ¬Ž?œ)I´Úa‹?—¬$eªn.?œ)I´Úa‹?ï@ñ'á6ù?©í‰éO?—áÍ£Ù!?©í‰éO?êÎ$P'ÙE?°é[¹É—?ÄÇn½´šì?°é[¹É—?íÃÊi1Å¿?˜ÙgÅêÆ?±á¬¶qÒ?˜ÙgÅêÅ4FGL J2216.9+2421¿ÐÒY¥'À:r¥'ÛçóÀ9†B"ÏÞÀ<*4žm>@oâ~9ì¶@é©¿Š¯?²˜;J®Ïâ?¬uüº?ø·…Ýúòz@
°ÕöA:¿Ò}ÆUˏ¿á>Ÿ&Kn¿å–¢='¿ãh4çÌ-¿ãîª!üÿð¿ì…ΫÊÆAGNbll3FGL J2217.0+2421B2 2214+24B?ïû›b,®S?:"æ˜ß_?A'wMF³?:"æ˜ßk?ïý©?LóÏä(·?0‹³'?LóÏä(À?ïê2Q	ùþ?lúUbXÉ0?eÍ®ön?lúUbXÉ?ï÷Ç
;h?>eü·Þ?Pqïå‰0½?>eü··4FGL J2218.6+1941?Ù<®É"óÀ>P;€AÀ:ß!5Ú­`À<L½}®'@˜o¢û@V	™Üµx?Î
	}Ø
?¶$ø¡«¥¥?âÙ`>.8ø@´4¥y!¿Íg³BW¿Û•=׿és¹jð8ã¿ám —d¶¿ïÿÚpú>?æÓó! 8ÅAGNbcuGALEXASC J221854.64+193841.6?ïüo?ìè?:~«
Ú?<ƒö˜À·?:~«
€?ïõ´ÃéÏ?n7ºvYv?T—Äx,d|?n7ºvYp?ïn®}Ú/?‰ÈD­¸Ö'?¤T`‰t?‰ÈD­¸Ö?ïïd,Sz?SŽ)œšý?`é›Ó¬…°?SŽ)œšù4FGL J2219.2+1806¿ãr"'é¾À?¢i'ÄÀ8þÏ;<1À;×Q!ZÛ@¢ª‰Uÿ'@l@šú©?©¦"Ô¸Ôr?µh¯‰â@
¾cb¥ç†@"Êb9[¿Î"¤)•z¦¿Ýˬ;\Í`¿ãü& ûù
¿ã@/€ Kпè|·áƒ=7¿ìbíç$AGNfsrq3FGL J2219.2+1806MG1 J221916+1806?ïû´ô™ÂÒ?;ÓªÅM?A,-˜ô¹F?;ÓªÅ2?ïýÏêFé?SScܗ?7™€­È¼G?SScܗ?ïµÿHi?ôÊ
zÛt?'€-ý%¹þ?ôÊ
zÛt?ïÿßßæ#>äÊæ:%Fc>ðsŒíÕ>äÊæ:%EP4FGL J2219.2-0342¿è®ËƓÓÀGfá`؇ìÀ9Ê©Hš¤À<*yØ32\@蹃ÄÆ@ôɅðoi?»Ë"?À. ý;)¢?ü6öl‡š@íèQ¸"k¿ÏX"¿åޗ¿æ·û"p=¿è§:¬Î*¿éÉc@—ë¿ë³@S'D¿íý}¿HÌAGNfsrqPKS 2216-03?ïýñJ'o?(j›Ñj?0u«oô{L?(j›Ñj?ïý¨M:"v?O- ˜®"ú?2½–+dN?O- ˜®"ñ?ïÕ¯dÃ1?r£üKËXâ?u(|͞hJ?r£üKËXß?ïý¢T¶?$
Oàµìï?1êíZK#?$
Oàµì¿4FGL J2220.5+2813?Úg»–ã}.À7ÝÀµgÀ:Dmî$À<z8Cƒã@ ÷X¼…?ÿ
ä)à¤?ÂÁòh½®¢?¥Ø£š¤\?ã¹
"BË?þ'ÒÐÇÙ?ïú{üР—¿è¬Ôÿ÷«¿ßd­ÿ'+¿¿ÜÆOo©Ü¿Øå$ýd¿æÄç=AGNbll3FGL J2220.3+2812RX J2220.4+2814?ïü­	Kïõ?3…B>™I§?:—µ €Z¸?3…B>™I?ïüXú#?QÿËÔÑ?=?Ÿè.áz?QÿËÔÑ?ïñ¤3+ôy?fõPÊl‡-?\·™¨x?fõPÊl‡ ?ïÁ<Zœ˜"?eâfF¨?aÒ±³¶D?eâfF¦4FGL J2221.5-5225?ß8çJŽOQÀJ1	á*QãÀ9vvü¶ŸdÀ;ñžbeP@üDËaé?ù½R;66ô?°«¶ý'¢1?ºˆ©t
n@‹"ÞQZ@Öjˆ	#j?Ö\_ý@²ù?ËÙÂ~•1U¿Ó¹Ššù*¿Ó«<äâÃ.¿Þ Ý%	¤Ä¿ßÝD>HeAGNbll3FGL J2221.6-5225PMN J2221-5224?ïü1‡ç?9 Wnˆ??#†sÀÍQ?9 Wn?ïñ¢·©ÌÀ?"e\	xš?\º¬f'J?"e\	xš?ïÑÂV¦ø?|?ß×U™?wöÔ¬"ß?|?ß×U™?ïå
6:ÆÇ?Vªˆ×MÌd?jòÉÅ9:¯?Vªˆ×MÌg4FGL J2221.9-3504¿ïÁ£mÿ×ÀLžÁ~ºñÀ:ÆùáØ͌À<§¾Ê«Š]@û±r(f|@}õÏ$•á?ÉìtÝÍ{?Î3†V¤?÷E¶ù%ñ+@­ÇÜMj?ïþ[Ï߿⿛L4¿çîYyîÙg¿ìîiÀ
 пøÌ?îÛ@Î&i AGNfsrq3FGL J2222.3-3500NVSS J222227-350942?ïÿ9Mô¹à?!á€2^Š?ÖAhÄ£?!á€2^²?ïý©–†i*?OŒõš?2³K̶®}?OŒõšö?ï9õ08(??D\E%?˜ßYøúí??D\E%?ïü«¬Yƒ?2wàh"x?:¢Ÿí3á(?2wàh"Œ4FGL J2222.8+1209?ï¾îÕUÛ»ÀBWìÝ
Œ°À:c5*"8	À<8wškP±@¤ÔpZ0"@/MzÝð?ǜ
b.žN?Ł柆Ã?ü!¦ä÷·@T?b¿â½/k'–G¿áÎ耇yÜ¿åƒ) b`¿âя–n¿ïõ´yÒª¿ï}lÝxì{AGNbcuTXS 2220+119?ïøi";õH?QA\ã1?NY³*á9?QA\ã1?ïýYIs
•?Mô^Â-?55´g"W‰?Mô^Â,ü?ï{ü,t?‹uÌ@.8Ã?Ÿ }zq±?‹uÌ@.8Ã?ïæ¾Fî¶÷?\,—ZSú¸?iA¹I	j?\,—ZSú»4FGL J2223.0+6746¿íÔ\fl#@!©Õ<ÝÖàÀ:~?Àà/€À;Ú@@aïß@dða|qÁ@K³ŸÕý?ÊÜøHр?½û
wÓ N?ò_V§¬Ô?ö"hëPñ_?ïî}†¸–¿ç6geiç$¿åý·³àm¿å  †Þ+¿ð?ïÿÿ)@k*AGNbcuTXS 2221+675?ïë~:I	?i–ZX	Ñä?d~Ŷ÷?i–ZX	Ñä?êUô1kh?Í·'°¥¸3?ƨ-Ë:R_?Í·'°¥¸3?ímïÂ+þ?¢û:Ƶ^²?´‡î ?¢û:Ƶ^±?é<¡r‡/¹?´F¦>5:d?Ë
z5ãA?´F¦>5:d4FGL J2223.3+0102¿çW1öÿÀFMa€M˜9À;>Õ'åÀ<‹wI¹L@ Äkq=/?ü›Þ'׶5?Ñb
-€l?¿¶«G—?ñÞâ^.‰€@é£È¸?çÃ_›q
.¿çXÛch…%¿ãØMꣿÇÍ×0¨ê¿Ý·R<7馿Þ4hݏÖAGNbll3FGL J2223.3+0103SDSS J222329.56+010226.6?ïþý$í²B?K3™æóQ? -±$Ûê?K3™æó?ïþõBmÏ?K÷PÝEÿ?/ «Ù#??K÷PÝEÿ?ï÷&	—÷?\=¸Å?QóìÐ?\=¸›?ïóø6p÷?F"mG7¼?X"àG?F"mG7Ì4FGL J2223.4+5814¿æhO(q]1?軈!!7ÞÀ9ƒÝòŽþ5À;'éÃ}˜²@ºµ ¶Cs@Ù¶3kg?ÌÜ9|Mƒl?Õâ‹ûÌ>²@é!S6ß?éðŽîoß·?ïûøi2Ɂ¿ãç—¾Vè¿çðSà&ñ±¿ï6©	y&¿ð?ðAGNbcuSSTSL2 J222330.04+581350.9?ïÄñڙ©Ê?­˜:Ãøu¬?}‡³+Ã?­˜:Ãøu¬?ÝæEŸŸsØ?ØÌՉ1Sæ?áÝ00F?ØÌՉ1Sæ?âåʈF9?µTq"Œ?Ûî4jïs?µTq"‹?¡B)±$¡?–1‰­kc?îëÝdíµí?–1‰­kc4FGL J2224.0-1127?ï!h€9JºÀJ­>'À;X"üS£À<m
Ø/×^@¹¡"I¦<?ýœ>	P
Ú?Ô38üö¶*?ØÀyJ]@4…]¢r†@Fg˜jš¿ê6ñL¿ëk»À5Ö¿Ò\rœª›¿Û×£TY¿é4ց+Ž¤¿ïV›LøWAGNbll3FGL J2224.6-1122PKS 2221-116?ïï<œ/Úã?d"tÂ?`ÃcÐ%ž?d"t½?ïôqŠ©fÑ?€I–òÎ?Wê­2[R?€I–òÐ?ïêø[ã?"ôŠ"§?žâ üԃ?"ôŠ"¦?ï½<	×¥y?rÚìð­(?€°ýŠ¡—?rÚìð­+4FGL J2224.3+7737¿àÁ¡ÕÔW@1€¾×@ÄÀ:yôºQ À<Ó'¹¬@*CÜ΢@ˆE~R?Øb«{™Sy?ÜÓ¸#rué@ÊÊ¡yaì?ü¨pÄä &?â{à­Tb¿áʁ=­4¬¿é1G ¨"¿íè?÷g¿ãŽYÊv±¿ïÿÿ>¹úAGNbcuNVSS J222721+773319?ì-÷my?Àq¸í)ޑ?¿ND—T0?Àq¸í)ޑ?æñ,¬rY2?Ï>ŒlÁô?Ò¦§Mœ?Ï>ŒlÁô?åöRËG?º&LÔQm¼?ÔÓZiqû?º&LÔQm¼?é¿é°¶?¶Ü¤î jG?ËçýY=&?¶Ü¤î jG4FGL J2224.5+0353?èÃðÖ
ÀEriƒQX¸À;`P‹2ΉÀ<ž>xá"@ ËÕ§½?ýÞeæä¦?Ð#$< DY?Á>ڛÂhÆ?ó&eYöì[@'Ãfœ—%¿í²æ§ieõ¿îEÊ¿×Eø?ïÿë""i·¿æ
Yº†y+¿Ô7ü:ù{,¿â¯má"ê¶AGNbcu3FGL J2224.4+03511RXS J222426.5+035445?ïþw<¦v?#?\gã!¹?(Œ5˜ŸÓI?#?\gã!¥?ïþEßýÎR?C0å."¬?+¢#àÓ?C0å."¬?ïÛ~p¢
B?x£ìbÊ?r@Ç®ù^@?x£ìbÉ?ï÷ÿDø?CÔ',?Pývã£?CÔ',!4FGL J2225.5-1114?íº´'ÀJ"Ĥ	_$À:¨ÝÛ
À<OÐîš|î@ÌÁën ?÷@]Øù*ú?á°Þ1Î?â5~†mÃ@ïƒ9@ØS"¥å¿ï;Wú'ص?ïí%HzÿåŸ/ۏÞ/¿Ük®Œp¿ïÿÿ" 5•?ïæ0¡¢AGNbll3FGL J2224.6-1122PKS 2223-114?ïù§1¤Z€?[RŠß®CQ?Ic9n•ÿµ?[RŠß®CF?ïõ³éäK‡?pfEVŒÎ"?T˜,7hõ_?pfEVŒÎ"?íæ&¡òã¥? ^O|½¿?°ÎÊðhâØ? ^O|½¿?ïÝwä3Ö?kr®
N'i?qD
æ}?kr®
N'b4FGL J2225.6+2120?®ÀÓ{˜°À>ó^1
¿À:\‰mÒkÀ<.2$?zi@Œ9j.òÝ@4ä†&ö?ŝZ³Ê?ÑöJ>ès@"éèwM@	¸§áÛÒ¤¿Õê£	"¾¿ç˜¨"HK¿é¾Ðà­ªH¿îš¿^z4¿ïò$_°¿¦?ïw:ÿ°NèAGNfsrqPKS 2223+21?ï÷ÂQ>òC?Yš¶À8~á?P{]'}"?Yš¶À8~ì?ïÂc´Š?™¤D' °?~ôÎ%ºü>?™¤D' ¯?îf©óÒ­?™Ž(%µµ?©Ÿõ`ÂÕ)?™Ž(%µ´?ïŸEëÖÝH?xšeaTT€?ˆ.…
H®n?xšeaTT4FGL J2225.7-0457¿çu!ÔÂÀHjœýÒ(VÀ9θ_WÀ<
¥T¸¾ù@š"ÀC§u@úÑÂÕÓ?«Fg~¥ˆ¡?´QVßµ²ª@—9~¦Ï@¦Mhky¿ÃöXak¿áâÈa®Û¿æÜrÒ¨"¿äØ`^'i¿êTCƒãNï¿ïÿÊñ*z'AGNfsrq3FGL J2225.8-04543C 446?ïýbZý[?-â_©¤—?4ïÍ(0›?-â_©¤—X?ïüÂ!-Ñ?VJ`'/?9îö'wÚe?VJ`')?ïͧÿJ¥»?us#õ*ã?y,Z­"Â?us#õ*ã?ïÿ-Ç南?°ä•
?GNM?°ä•
è4FGL J2226.5+6901c¿êÇЈD¼@#mfŒ&À;L‰~™cÀ<FdÆ@"퉰ÃW?®ìc.è:?æÚU웟-?ïþÖ¿ê¼!@¤Œ;ã@¾i¼²"?è0Ì ?ïò솦wοØö™NðþÛ¿â?Ö¿¿É?´ß´°÷.¿ç|<[Ðá/AGNbcuNVSS J222625+690207 ?îØÇêz?¡@¶²TìD?£ÆsXb?¡@¶²TìD?ïÛË
%¾?"Qü¶e¢?rzí ò`?"Qü¶e¢?îD²OÜC?l·C¡?«´Û;Îx?l·C?ïÅgž7¢X?|©	Ú·?}L0ä.Ô%?|©	Ú·4FGL J2226.6+0210¿Ø@àÏÍÎûÀF;€Ü3rÀ;Y.yÖÀ<…¦Ž@!¸IƯc?ûÓµõó?Ì^ív:™Ú?¶&	>˜7?ì%vå@ú5ÏÅ¥'¿ìÉW,6À¿ïÿóÖ&ã?ïÿꁺ¿à>"7Z	¿à	bŸ‡oK¿»'®îÀhAGNbcu2MASS J22263636+0210373?ïÿ©¬/=É?$_U>
?"ô0¹®?$_U="?ïþ®2MÆÉ??g'¸ò`?%Û#"p¿??g'¸ò>?ïõT½±{p?f¢"{ۙƒ?UV"	¯?f¢"{ۙ~?ïüEtm?3ñÍ;zÌ?=Ô_û}?3ñÍ;zú4FGL J2226.8+0051¿ï®£YRH"ÀF°CécÜÀ:2lÙG."À;á/Ø4ßÜ@§¶¶@F€d?ÃßÉi@
‡?Îz°m¸@Œ:䜸@×æ\ÀË7?ïÈzW´ò»¿ÀÐâC5à¿éaJÓbé¿ç޻♽¬¿ïÿŸR@>´?ê1þ –
AGNfsrqPKS B2224+006?íuò§‡³‰?·íx8úñ?´PjÃÂc±?·íx8úñ?ïî`9Ð?³®1W@9?B?øÆ"?³®1W@9?ê@X[Ÿ?­™5ä±^?ǶþŸö''?­™5ä±^?î4Ÿï™?šcáûÑ?¬¶Ï`?šcáûÐ4FGL J2227.9-3031?çˆv(‹ÔÀMAð€0<À;n4˹§VÀ<ØYí²¢@ ò0´}Ì?ÿlº=~?ÊYÐ@tº<?i6+»W?¡±‹OÈâ@®©ÌĿ¯ÂÐË?èéÅ+Û¿¿Ö@£[å.¿èºÿƒ¿ÄõÊ\…!¿ÚÄ^Ô¡­dAGNrdg1FGL J2227.7-3036PKS 2225-308?ïþr¶º?1 éJÇ$?.îԔA;?1 éJÇ&?ïýöExµx?VR¨RÅ?0MÔ:TC?VR¨R¿?ïƝv%?|¾zY¬?|±Dí¸®?|¾zY¬?ïþ·j3%î?'_\ÿ$?$‰\Í¡ ?'_\ÿw4FGL J2227.9+0036¿ï©±Ÿ¡³½ÀFÞùü°À'À9®GE8ï5À;Í´ÚgÀ@B89,qx?ÿNlªMF?¶
ï×¾ÃJ?ÀB}þÞlÝ@	†)vò@&ם`Mž?ï–<¢¤@¿Û¥oÛÛ£¿Ù²¬…Y›¨¿ÙÕyäÈl¿çr4/²u3¿Ýí¾Ÿb†]AGNbll3FGL J2227.8+0040PMN J2227+0037?ïê»ùŒC?h	
"'?eèDs½?h	
"'?ﯥÙЛá?¢'r7՞?"‰‹ÙÕ?¢'r7՞?ï¥æJATd?†˜qa}=Š?††moªç?†˜qa}=Š?î£v@5ò¦?¡]î°ðP?¥È›ü Õ®?¡]î°ðR4FGL J2228.0-4155?¶ý>ÀL¤ÿiKÀ;Óúú݁PÀ<ö[ªJÁÅ@!ø-ƒpã?ü'/"R	¸?Ð`û£$ð?´ñZuÂNï?êð¾'d@fRðÜ¿ïÝÜ>¯¾?Þ?»Ø?ïʵe§ú…¿çÒ¿?›vi¿Ës˜=£úq¿ÏKi W£ÖAGNbcuRBS 1864?ïÿ5XÁU?ô!¯¹?TçÕ]¡w?ô!¯5?ïþ®ºTL»?@NÿÑÊ×?%Z»4IÕ?@NÿÑÊ×m?ïÄBéÇN
?~›OD'^?}ދXú†?~›OD'^?ïûÛt:»
?7+ýцš?@'/ԛ?7+ýцš04FGL J2228.5+2211¿íMÍÈc}À=ÊøzЀ¶À:v×ÁóT÷À<Q¬Ô	1@ë9¸2‹î@A©¸ËŽ?ƪ×Y˜¢¤?Ãõµ¹µÃÇ?ûPÔ´!Û?ü«H%2¿p?ïô›?¥¿Ô6«ÃgÉ=¿ÛRDËáë¿éâd®ÖAÁ¿ä‹*5]¯Þ¿ðAGNbcu87GB 222614.9+215540?ïfæi—ù-?""rH§?"#2Íڊ?""rH§?îìÅiÄ1Ü?¯Y9z&Í?¡3©c¼âG?¯Y9z&Ë?íɞðzߗ?¢l9²ç¸?±³|)N?¢l9²ç¸'?ëÇÿ¡H?¨?ÐNæ£?Ìà…zá?¨?ÐNæ£4FGL J2228.6-1636?äå–ȼ
ÀK±#öM¾À:m›¨g'¶À<xÐÜüŹ@¿Î´-™–@?'yꧩ?¾âÊ: bK?™l#"¯¤ô?ܶe§"ê@²¯ï;¿ë¬k˜ÕN|?³'«hÎös¿Û†Iû̔™¿áðk֙տãȓíˆ.7¿ÚÖ Ř%AGNbll3FGL J2228.5-16362MASS J22283018-1636432?ïþ3­J¢·?%gO⏟B?,Å+UÔwð?%gO⏟?ïþu2úä?H±=w²<?(¬Ð^¡»©?H±=w²< ?ïñ"K'œ?g/ØZ'*?\Ùi°äÈ$?g/ØZ'*?ïÿ)@¾*?¹¸‰%¬î?×è:®?¹¸‰%­š4FGL J2229.1+2254¿ïPdõ(- À=M5e<š»À;€€ÃàÀ<ž£;M@ ôáÊà¹i?ýá©»Þh?Ép£×
=q?¢%¹øߥB?Ø:€›k?ö¢<þ?ïü±a6{½¿ã9 Š¤‰¿è»ÞÓ_Ž¿Ð"L€a9V¿áÙ|"MÀ¿Å\Ùê¦ÒAGNbll3FGL J2229.1+2255NVSS J222913+225511?ïþ_¼œ?O¥Hǘ¸?*"?æ<A?O¥Hǘ?ïæ<ŠÑÒÓ?€oá,'v?iÃu.--å?€oá,'y?ïæ¢óDF÷?pŠ]¿`È?i]»¹
Õ?pŠ]¿`Å?ï~ÎnØRð?x ¨C;¾)?&2$õ¢<?x ¨C;¾%4FGL J2229.2-6911?ÞÖ[8º¿êÀE	 :2+À:–(òÀ<~•rÃkû@ÊIÞEp"@_þmXÉ?¼L^}cØí¿©"¯#æÜe?ì!$þ<0ˆ@æ)ë
û\¿á¸Dêë›Å¿ãB;䳿æ§Êêt}€¿å'Paí/ï¿ê÷¢cl·¿ïÿ¦¶tFAGNbcuPKS 2225-694?ïíJgácI?a$ƃWè¬?bµ˜œ·?a$ƃWè®?ïôA¹?o·" ®?W}ލùƀ?o·" ·?ï­ñ{à[?ƒU	dàéO?"ƒ¾!éZ?ƒU	dàéQ?ïÚ»ö%Èý?a™»O»Ãþ?r¢í›?a™»O»Ãþ4FGL J2229.7-0832?ÐB/*€–ƒÀIÚÃ.¾YÀ7㸫­˜TÀ;¸<ù…'@6r$àŠ@ÉWòÓÈ?•ŽšPèj?¹^¸`óϊ@þU@ÓfI`I¿ËU+«u+¿äœ.܌¿è]º|h0¿è½¶ÿÛíÒ¿ìÀ©s+pÇ¿ëêM`ÛâêAGNFSRQ3FGL J2229.7-0833PKS 2227-08?ïú_<öëN?e,vëL N?Fƒ$RÇÒ?e,vëL N?ïíw!÷?yYsd&,?bˆÞ<Hï?yYsd&,?ïhGÏR)?›íUOÉà?'÷º¼?›íUOÉß?ïøLý¥þ?B÷~q?NÌ	h…p?B÷~_4FGL J2230.9-7815¿î®×"ø][ÀB="V!uÀ9ü›A9†4À<NB€Æ@$y&5@*t:dÜ?¸LêijÓ? §½sñó?ääýp-º@
›™pÿÇv?Ú¾..½¿ã²xÞ8/¿âhrzpßf¿åã¡$¨Uõ¿àyâš'¿ïÿ¶cÔ»¯AGNbcu3FGL J2230.5-7817PKS 2225-785?ïû|H×»?<'ÛãE¼-?BÜ¡½ï?<'ÛãE¼?ïþ÷†°?I)"ÊÁ£K?.Ї—$ùÂ?I)"ÊÁ£@?ï۱ْ,?t´SS¯ï‹?r'6éøÜ?t´SS¯ï"?ïùÑ ÄÇ?9:f?Ù6$?H»|íˆâ'?9:f?Ù64FGL J2231.0-4416?íîÞr7ŒÍÀL5'Ì÷À9ÓÖxG9zÀ<†óEšN@tu%Çe@8TÛ#§¥?±vp_8Ÿ¯?¨œêB9Lj?ðxë¤(hÕ@,(¡3ìÂ?ªÛk¡
×.¿â}5´Âë¿ç "¦£m¿æðÀ'+ç¿ä$?	ˆ?¿áüâ©­ãÓAGNfsrq3FGL J2230.6-4419PKS 2227-445?ïÿ-Ð.L6?]2EÐÀo?Eú6y;V?]2EпÞ?ïþ›ŠWò?AúÂ@o)?&G^j€ÙM?AúÂ@o"?ïíZ¶õ±¤?b¥bݏ€?b¥I
N\ ?b¥bݏ`?ïÿâ< z'>ãjóšƒQ>íÃ߅n>£>ãj󚆀4FGL J2232.3+6246?âa«p8@G"#ρÀ9¥s¶±•À;M`ÈW@b$uÖÿ@Q*Dw(V?ËE$wX§?ÅÍ£À#@w]š
_?ü…ktm:@?ïÿôa¼2¡¿ÚlUÿø¿è#†b/J¿åha}ÉY{¿ïüG¿e ?ï'[>ê÷ZAGNbcu8C 2230+625?înò¼2Â/?°'í¼½iÃ?©Ô<ÓÝ?°'í¼½iÃ?á…Xž§ÿ?Õÿ X}¾?ÜõN°ï?Õÿ X}¾?å'ý®¬­¤?·O©È?ÔÚ¢¦¤µ?·O©È?ص¬(¶?½+)Ý¡g¥?ã¥r)ë¤ò?½+)Ý¡g¥4FGL J2232.6+1143¿ÜôB'÷ÀCJ¤ÁëÈ;À5pP‡×ÐÀ:{ô°@¥@ÖÁmH-@–™â"µ.?yW§lý¤?µ^¢¢¬½¹@9–x?'æ@&sg»Ðü¿Ë˸e6»~¿àf·#îÒ¿ä¿ëþ@bF¿äGÊß·¶¿é®‰`‹é¿ì¢úkkˆåAGNFSRQ3FGL J2232.5+1143CTA 102?ï•HlJ'?‹Û  yŽˆ?Š­äÿí_j?‹Û  yŽŠ?æ_P¡%ª¸?Ùý°[–‡Û?ÓA^½´ª?Ùý°[–‡Û?îABX‰´–?¡~³f{Z?«ëÚwd¶‡?¡~³f{[?°/)Çyª?µ
zà?íúÇÌJ?µ
zß4FGL J2232.6-2023?î;50¤,æÀLÓ²VÿÁÀ:ä#åGîÀ<›OÚ2æÝ@ 2ÀD©'V@ÒÁ&¦]?ºz#À8•¿³"F|s)?ù/JUŽ§Î@P@à'¿ÂËr"¬Í~¿è¨nÿ<5»¿ç¤Z¬1¿ÇͼŸ9¿ÜÔWZ¯Îå¿ÛLyÊÇ9AGNbll3FGL J2232.9-2021NVSS J223248-202226?ïþ^ííX?&°‰‡[Nz?*!*~(?&°‰‡[N'?ïý¸=ŸEp?F"ºCmS¯?2>Ô}«?F"ºCmSº?ïøã¶Þãœ?RáGFåǒ?Lq$"q†?RáGFålj?ïøŒŒN­š?@Y#/AZü?MÍÎÅI•?@Y#/AZò4FGL J2232.8+1334¿ì:ð1fÀB›3ÁÎl	À;{]š
_À<»£IEÄ/@!§â^¯bÚ?ú¯4^¬^?иn¼ W8?¾õCŽu#C?îõ'àh@žwNëö^¿ïþ!¾–©$¿ïEHßlâ?ïÿùëñ¿ÍAÒ2g[Y¿àÔ£éտ̇é­WAGNbllRX J2233.0+1335?ïÿˆƒð?ÛòüàU?
Ü¿_Éø?ÛòüàX?ïþ{§Œ·1?Bփ+Ð=?(E‡4Œó	?Bփ+ÐK?ïõçø©?`Þ)L¦?UÖ1ö¯?`Þ)L°?ïû°|Vw¨?3ÞÖx¡¿?A>¦!_'?3ÞÖx¡Â4FGL J2233.9-1229?7¤æÀKV®Bž
BÀ;"k"ÌÐÿÀ<™êBÿY@=^ú·@É?þyòoÀ?Õ<ÿD™7?ÌÈm×ôÉ?ôré+¨$?ý°|Ҏ'º¿ïᕱ­Œ–?ïöUç¡9¿Û(øýWY-¿Ü!YÁèBI¿ì‡Ø¦õ¢¯¿ïÒ@tdUëAGNbcu3FGL J2233.5-1235PKS 2231-127?ïéç¢1zœ?eáÿ—<öM?f]΅cà?eáÿ—<öK?磻ìÛ?šÐ㮊 '?†–Äø½	W?šÐ㮊 '?î]V§cÔû?™¥ûÇze?ª*•‰Â°W?™¥ûÇze?îË]Ãúd?•«oÐÿV2?£NJ#ÀY´?•«oÐÿV14FGL J2234.1-2656?ïšK:€(ÀMî£À9F®×ï?¾À;ãð/¨d8@>|ÔçÎ[?ÿF7õÿÌ?¬¹¤?ԛ?²Râ¥üÿE@4†º™Äb@[ùëñ¿Ö9Tç¸á¿Í6ºý–š¿áÃ^6=¿à÷ÍAìa¿à¿ÓÀí¿åÚI{«AGNbll3FGL J2234.1-2655PMN J2234-2656?ïÿ:?«ây?¶JÑbÙs?¸
ƒ°Å®?¶JÑbÚ7?ïþ­6¼?J¬‰æÍ°X?.ÏÕ,"AB?J¬‰æÍ°l?ïÌkdz?zÖ:ÑӋÈ?yôÊMüB¸?zÖ:ÑӋÉ?ïÿÒD{›>îDK#äÂë>öÝýB1ðC>îDK#ä¿<4FGL J2235.1-0623¿íô;‹r•TÀIʱþë-
À:ßó£Ñ+À<"ÇÝyÃ:@ãܚJC›?ðà"¾ŽE©?Ûy—¹>Ð?ïm8bGõ@æl£—I]@ä(Þñ¿à¥TþŠ	.¿Óiû±¼¦¿ÚÿÔač¿Ú®b¾ç	¿ð?ïÿÿÊPËAGNbcuPMN J2235-0623?ïù·ÿÖü?S›ͤS?I §è±?S›ͤb?ïû¹¼i'?[¼Âáæ;2?A['¿m?[¼Âáæ;G?í¿Ú
½l8? Š›TëÈÓ?²/'ž3? Š›TëÈÒ?ïô#tv?Wj"¦j@?W¹ÚÅÑ?Wj"¦j@4FGL J2235.3+1818?µu¸Fô|À@ìƼèS;À:i"6ÆÀ<h·'"…@ğ+ÔÅ?ÿƒ†Üþ?Ï¡Ñv¹?ЙäB4Wö@RóݲÎ@:äßJ¿Þ®ïÔ;V?ўY<1^¿ãÜÝ¡0fпÔ<_p#¿ìaÈ"n·¿ïÁmž%øAGNbll2MASS J22352860+1816356?ïÅ
hÌF?<ô?ç?}yu˙Üô?<ô?ç	?ïõÌíV?lái»x:w?Tf%Å×UÌ?lái»x:u?ìI'ƒ\R[?§T׃¦·?½¶Ãåm$?§T׃¦¶?ïw«Î…Ô?}|ҚUê[?'
†/E}¿?}|ҚUê]4FGL J2235.3-4836?Ün;yŠÀL
×6&-À97½8SLÀ<YÑ쒛@¬Ê"ùT?@o`àëh?¤Ý,ÁT¹?–ä&¹/ê‡?æãôÑΔM@Ÿá∠οÝR°[Ò䔿âÇZ!‰'¿èý'¬¿å"]àZô¿æ4²G^¿áHrÏCAGNfsrq3FGL J2235.3-4835PKS 2232-488?ïÿz{ˆ?
JÉi?¿}0þ?
JÉh®?ïþÁ˜ô=K?@«·Côsé?#æp¼+UÃ?@«·Côsß?ïìBÆÅñ?`Œ»LrÓ?c½9:âô?`Œ»LrÆ?ïÿ›CÈ2?*VÒ2Øc?	/
ó[™Æ?*VÒ2×Â4FGL J2235.8-3627?ïñ"GJ°3ÀMórq6¤À9}'OH<°À<\²ò03¤@§Íęw‹@Qæ­j1?®Ø\fÍ?³©/¶@ð{xFb»@
C+ò!?ÝC›=]¯¿áÜ®ÙÄ­¿ãOx¶Ë¿ã	U~·–¿æ`ai§d¿ïýüðüAGNbll3FGL J2236.0-3629NVSS J223554-362901?ïþ1Ÿœj­?*H~E?,æ9U?*H~n?ïüÒeFp?SŒ|?9lÕÌæö?SŒ|ÿ?ïÓôe½?y›-FWm¾?vùÍ Ñ?y›-FWm¾?ïéãÐìØ?U̳邓¯?fø/'+?U̳邓²4FGL J2236.2-1706?íûµ­é
ÀLŸºˆ&ªÀ:'Û ¥&–À<k—€º¥ƒ@øےbm³@›ß>¿Xp?¸2Ó	'¦?¹•b?äض%ö@<ŽP».?ìÎø@n?¿Õe;Ãûm¿ãÝK8)'¿äúm^Ó!¿Û9æ@;Yr¿ç—ͤ?»AGNbll3FGL J2236.0-1706PKS 2233-173?ï×äþ϶?nm0î\º?t
€¸¤ä?nm0î\Á?ïø~¡û/€?`ôOD4?NxBj?`ôOD4?ï€'ÃSb?Šj_äÛÜ?ûO+'|?Šj_äÛÞ?ïÓ`ÇÒ?dac' ?vOÿœtÄ?dac' 4FGL J2236.3+2828¿á¥ef4¥ŒÀ9¦M;òõVÀ7Éá|‡:À;8œÿ¨@k'HíYµ@*ˆïþ*=?˜N𪢀?ºÄñŒܺ@ Ú£ßm¹A@@Gbj-p¿À¨c¶Þ£å¿àz¡†Íå¿ãwœ¹ßŠ?¿æ#… êÚ¿èqJÝõ¿äy®ý®ìèAGNfsrq3FGL J2236.3+2829B2 2234+28A?ïî"âéÑ2?d`í§Kì?aÝ.Îx?d`í§Kñ?ïé*$ ©
?zÀi}ê?fÕÛ_Vôe?zÀi}ê™?Õ2X!?ˆa°I·úÊ?‡ÙJ³i÷Æ?ˆa°I·úÊ?ï̊ˆ	¬Î?j5k\IKš?yº»û)˜Î?j5k\IK™4FGL J2236.4-2309?ɟìAß1£ÀM¥ÈÉ2
™À9á^"ð•)À<drr
c–@l#¸ìÆ@P%çñ?»D?JÑ-?¸ŸŸ˜O?õ2cʪ³@uåµQ¿ãSe¢òð¿âµl]÷,¿êž€‰'\¿èl7`¿]¿ïÿpŽ• ¿ë@ðàþ2 AGNbcu3FGL J2235.6-2319PMN J2236-2309?ïÿㄷs?nQðQ'?ciÊÉ?nQðQÅ?ïý¡ÿÐHà?PC~Ç¥2-?2ð}¸ú¿?PC~Ç¥27?ïßÎl¦í?pVc'¹*K?püI¬‰þ?pVc'¹*N?ïø~üš07?ATÎO€wD?N
—?Ô?ATÎO€w<4FGL J2236.5-1433¿çA¢hH©™ÀL›ºÜ	À7™šFgÃ^À;R; g@Úô	Q¸Y@"3ÿ
z?–A…s"?²-í_O¬ø@Ï⾦™\@çv¹iÄ¿ºþÜ>"Ë¿Ý 뽨¿âÔ"Œò¿⹁@‡Y¦¿æ€ƒ}Îaø¿èי¿"9áAGNBLL3FGL J2236.5-1432PKS 2233-148?ïøàãv¨G?P¥ÕL?L|r%^Þñ?P¥ÕQ?ïñ¢ÓÇx?~ÓÞ¾{?\»Xqt?~ÓÞ¾~?ïÔ\Ǹ
c?|AÅaZŽ?uќ#ùN?|AÅaZ'?ïÿ¯)F¾À>ûDEZ–ÐS?5®PPG>ûDEZ–Òƒ4FGL J2236.6+3706?ä,8 YÀ2c¥]:ÉÀ;A¹'ÔZ`À<šE'±H@!þ75Ì?´?ü<b¼ºh?ËóÍ–&?˜ÃOܝ`Š?ÏÃYª¹Ò@k,†›»?å!͗¿áìv0í¿âeˆðÔê¿ã<`®kŽ¿Ëßõ½‡¿Â"3£ñaWAGNbllNVSS J223626+370713?ïÿ‰ 
÷?	ÚoØ<?
·ýB>ìx?	ÚoØ9?ïÿŁik?8ø•H[y6?‡OÒÒ½´?8ø•H[y?ïõ¶Ôá]'?e3­T<?T'V=DÜ?e3­T<?ïýye@§þ?,ôõÖ75?44ÕúÀº?,ôõÖ7R4FGL J2237.0-3921?êF낁ö$ÀMË~dž<À:–VîúÀ<ˆL×I''@léú=|@–Íl.ýD?·üß¶´]?µy™ßd©ù?ûÖÃƓÎ@՜9\-¿â¨+BNC¿â«ï§Ã(¿æ~¸—·¿ãÿL±‰zh¿ð?ïÿÿ>¹úAGNfsrq3FGL J2237.1-3921NVSS J223708-392137?ïÿZÚB˜Ê?¶=Ŷ1â?¤·¬æµ¹?¶=Ŷ2G?ïþÁ¡w?=ÉKäº:?#ç%è?=ÉKäº;?ïÍ ö"có?gx¬/ŒÙ?yo"¶N?gx¬/ŒØ?ïÿäD æX>èøªv)Ì>ë»ß¨÷e>èøªv.,4FGL J2239.2-5657?ÛÙÁèü_ÀJã—­À;o†§NŽÀ<ê>Ä`î@cŠ!+ž¿?þ^ã MèÁ?Ù%™A¯ø¬?ÐG¤"Y@Ž?ù–p4Eê?þï~'£2?ï²µ>»§‹?Š8=3<B¿â :<½¿á°ìœuìì¿ïêë I÷p¿îå[n»Ÿ~AGNfsrqPKS 2236-572?ïÀoÂú¸‹?Î_²Ñ–«?È'£ºô?Î_²Ñ–¬?ïºô&{¥?"*á}§?Böaº7?"*á}§?í'XE›Á? œ¯ö!µ?³m?Ó"? œ¯ö!µ?îñq2°Ž?±38\? èìÞd÷-?±38\4FGL J2239.4+5130¿énìu"À¾ºñ6;À:!K,F°À<N0å{@´Î3@*y]¹ïz?Ç!'al¯?Ó]‰Þe¦x@+‰>@+±ÐÈ?å+$;H«j¿Òë!Cœ¿ænÚs~|Þ¿éÑÇ"hà"¿ïÿÅ}M2¹?áEUt¦›AGNbcuLQAC 340+051?ë²JyKt?¹€ãÝXž?Á6ÖÒ4?¹€ãÝXž?î¥Í!ßÞN?»Q*Où?¥£-â?»Q*Où?çõNÛôº?±ºc"©Ðº?ÐbHè‹?±ºc"©Ðº?îD
¬Ä?–Sãuʊ¤?«¿.3¿'?–Sãuʊ¥4FGL J2240.3-1246?֑)ƒÚǃÀL
{é…jÀ;WÓpóˆÀ<Œå—ží–@ åp…ùÿ‹@?ßÁœ"?ÃCeÛQ¿¹µ	a¨'"?ò…Šƒ| ã@ÈæšSRã¿îéºy
2?ïœ&Üã›E¿ãŽñŸêì¿ã¶,ýx¿ßS€Èп¾`ÍöŸAGNbcu1RXS J224014.7-124736?ïòØoŒ+°?ZÄvΆE?ZO 稞Â?ZÄvΆI?ïô\ 2Ó³?s
D,D?WG¿šX›<?s
D,@?ïÑMÅ&‰?}ŸRšR'\?wvÙl»Ì?}ŸRšR'b?ïÚ[^0W?e©î¿åî ?rÒPçÔp›?e©î¿åî–4FGL J2240.7-4746?ë鍁gµ;ÀL¡R}ÔAÀ;Îj[¾mÀ<Íëýê|
@ð¼~ ïÏ?ÿÌQ—¢H•?ĸ[%À"?"bk¸"b{?Ð2ý›¡²@ÿtHQRƒ?ïjà"'¿ë£BÄ ®¿§ãØ_°J¿ãiÀùYó'¿ÙpÁž›a¿âÇP÷iX‰AGNbcuSUMSS J224042-474733?ïýØv…?,据Ûë4?1<O§SÚ¹?,据ÛêÓ?ïýҊ£lÏ?QîE¶?1kªä™Ž—?QîE¶?ïò@¯Aïy?cõ#‰1Ç\?[~¡|!N?cõ#‰1ÇM?ïúzÏ{û>?6;:J¢O?FÂ¥?6;:J¢+4FGL J2241.1-4122¿Í
a#Æ9ÀMä|"µÜÆÀ;úd­(—À=‹Ydö$@"'ÌGÂ?àZ«n®4?ë
¡äÁ¶?ïÿ ^¯¸À?þ¥nij&å?ûmQÇÈÖô?ï¢b€}¾È¿éªÀ2‹¿áÓ¦¥ñ–±¿ÊLœ»·ü†?Á.èävã¿æ)ù˜Ý±÷AGNbcuWISEA J224103.56-412155.5?ïìr–Ž"Ç?d_Ëlj?ciql:º?d_Ëlk?ïøº£î¨l?gsDþßÃi?MpE^Lú?gsDþßÃp?ïX+ú\v?'åàÚ\ï?"ú€½4q2?'åàÚ\ñ?ïâÐx<•>?q³á¸ð§÷?m/‡ÃjÁ?q³á¸ð§÷4FGL J2241.2+4120¿æ`œ ­òìÀ.bdä†&öÀ9×Ϗõ«éÀ;ç¼SØÅ)@Bðòç>@n?©c;?¶‹&å#ø¿gï¾d5Pó?²—Ð¸"±@wwZÕ?ëߟ¢È…¿ÌÖÒI¹\ƒ¿å	€¢&Ûâ¿àvé€â"‰¿âS¡2OB¿å2_ê pAGNbll3FGL J2240.9+4121B3 2238+410?ïìÃä6Z?\F~òz?c<Éæ¥ ?\F~ò~?ïþºXíE?@ìgôX?$Zq.«ºI?@ìgôX?ïÍ?X>/C?{çN‰Ïö?y`Sàè^•?{çN‰Ïÿ?ïð0£7m?LXgÃ	òt?_ž¹'%ޟ?LXgÃ	òs4FGL J2241.3+2943¿ç
-¥uýÀ91jœV|À:ÂðBóš—À<{""i·T@ q/ÓØ.Ö@óøUӍ?·IËù")¿·ó¡!ù$@Ú~<F@üU8k¬K?Õìmçd'È¿ŠðÔqlù¿å×4ó&Ô¿æä>ÙY£
¿Ò×'™¡ý?¿—Éà´5QAGNbcu1RXS J224123.5+294244?ïü><´®i?=‰Œ¡òÝñ?>ZŒÃ¨?=‰Œ¡òÝÔ?ïüþi0s?QöÇ=­Û?8¶|g?QöÇ=­×?ïÂMîÁÓt?¨a·xÀ÷?~ÙŸF.?¨a·xÀô?ïía(Ë?S¶_;#?(?bž×4ñêË?S¶_;#?$4FGL J2243.4-2544¿ïÜJ"µ¯§ÀN²]yЦÀ8ó犾4"À;·ÇHÿMS@TXD9ÀÁ?ÿú¨W¢~E?ªñ#
Ì?ÀÝU@w­_I;³@S¥m¼F?ïÿÀà/€ ¿Ù?e*)¿àaâއ	t¿ã+Ñà2_¿çÌéhM¿Ù€/»."¾AGNbll3FGL J2243.4-2541PKS 2240-260?ïß±9Û\y?uL†ñ²?p'cQÄi?uL†ñ¶?íÿiò?ÅÇ».tM
?°7ç°w?ÅÇ».tM
?îŽÔáW/ ?¡
5ʋ?§±ê?¡
5ʌ?íÕ²ÒñØ+?—
ŽtLJ?±Rihq>¤?—
ŽtLK4FGL J2243.5-3931?£AœøÕ²¶ÀN`:!cýÖÀ:‹ÆÞÀ< 7Ǫf@½ëf?úí@w❪?ÃQsûz_B?¼BÎÜãÆ?ö¯Äcq¿`@E3²_
W?Ŕ€ãÀ.¿äbžÍ¶¿å$¨ Eæ¿æy¦µ¿è%Áۂ¿ïýݱ žÜAGNbcu3FGL J2243.2-3933NVSS J224326-393353?ïýIÝî8?/cÔËmù~?5±Ž;õV?/cÔËmùá?ïüªR'uô?NüUËÆRó?:­nÄPf?NüUËÆRÛ?ïë«°%µ$?eR!†?dTOÚJÝ,?eR!€?ï筎̔°?T‡öÌ]?hRq3kQ†?T‡öÌc4FGL J2243.7-1231¿æXΝÄÀL_9&A³À:pûëžÀ<7ªËñ@žhJí6@‹SB3'?³ª$>®ç¿±±ß‹–K±?ý÷½#â]@~矕¿âu	—Xw¿éxHÞ½¿âD­Cš‰"¿ãS{ýýFg¿Ñ)O¤Øçã¿à³ã'/ßAGNbll3FGL J2243.6-1230RBS 1888?ïÐJÂV?vKù…"}?w÷ڞԿ[?vKù…"|?ïîÁÖ#óÔ?•Ô}*8®?a>)Ü-m?•Ô}*8®?ï¤Ö"£/}?ˆ5ŒF3?†Ê^×4 Ü?ˆ5ŒF3?ï×´#ç?dÅÏב?t%îqv¦?dÅÏ׎4FGL J2243.8-2510¿Ñè¨&t4ÀN¯'Àa"À:~-o}À<
qäHêU@M¾—@iÒaaCè?ؤó…?ïÿÕm…>™?üªáÀyØ@`œ¤ç¿Ôúҙ•gÜ¿â ç×Nl¿è±¸¿y¨
¿í•
È?Ÿ¿»{šâD¿ïûX0B½ëAGNbcuPMN J2243-2505?ïÖ*E€!?'"ًy"µ?têÝ?ïsæ?'"ًy"·?ïýu$Vþ?M\àè@?4VÝHëP?M\àè@?íܧ~m?¢›˜Gæ'°?·‰Ä—?¢›˜Gæ'°?ïó­êA^>?Tn"Í=µé?X¤+}C'"?Tn"Í=µì4FGL J2243.9+2021?ÇêK²p À@®÷S½À7ìõì€Ç;À;5ìlø@L·
Gç?ûrÀç¼<\?þÞmÅ<?µ®_4ª@qØ¥H#…@.G«æ"^?ËѺÀ/Û¿¹^f'±¿ÙrԞReþ¿ÛØz™9¿Ý¥SŒ¿âpY.oAGNbll3FGL J2243.9+2021RGB J2243+203?ïîåI:7`?F
…p¾Ú?a¶ÅÈ Î?F
…p¾Ø?ïç-½22>?|æ®ϯ×?hÒBÍÍÁh?|æ®ϯØ?ïÊet3?dÔ‡7?‹Íz&¢ó?dÔ‡5?﵅FÈõ?nÉJ¤n\?'ž¼îMÂè?nÉJ¤nb4FGL J2244.2+4057¿Ü1Xª¯¦À/šw@Ý@À7zw⏬±À;3R­Kþ@¿AùŸ"@4ìÁ^ځ?"œ˜ëZ?¸³7¥]È@$©?)
»@ »Çö|?¨+Ø ¿Ýh܂¢\6¿áóìáÀ#ò¿á0%⒱ɿæÉñ…é¹m¿èÏ|_LØAGNfsrq3FGL J2244.1+4057TXS 2241+406?ïè™Í–4æ?dkB~%f?gf2iËÝ?dkB~%g?ïÙ3V#›š?‹]vš‹?sfTî23?‹]vš‰?ï5üñ"m?"ìÀ¶ÅY?™@aÛ¿òE?"ìÀ¶ÅZ?ïü]h
M?;l½Rú·?=¿G­¢]?;l½Rú'4FGL J2244.6+2502¿Ì€ZÅ*ƒÉÀ=‹T~–À:ÆcQÞïåÀ<"PP@líañ3?üðiϘY?ÑÖï»dD£?ÒòõÀáÜÿ?ÿõ²ÉìH?ùÿ¥è¿å÷É?¤…±¿ÑÑðã'pÞ¿ÞçIeN¹L¿Ø£¹bâ£N¿äáâ¾P³!¿ïÿýF\IAGNbll3FGL J2244.6+2503NVSS J224436+250345?ïôZ:e¸ì?Tàø¹ó¶?WK‹4Ž'Ý?Tàø¹ó¸?ï² -X/Ð?˜ÊÍZ}1K?ƒWô©ô?˜ÊÍZ}1K?îüÎë]bP?"uNCD-? 3J)Û?"uNCD.?î	y] Ê?"Ø•ç[øÁ?¯hj-ÿsY?"Ø•ç[øÃ4FGL J2244.9-0007?ïN=_û†›ÀH­Üa•FNÀ:ìj`Æê5À<CãÎq»@VU7«@pÜ¢b–?Éç¨ìMñ?€}:	Þr‰?³¤ÁÀÕ?ÿÞ½:2¬?ï*2‰}ÿæ֙ŸxÖ«¿â^éÐÒk¿äjÜs­¿åcŽz¦^¿ïù?A3|AGNbllNVSS J224448-000616?ïøö¤kew?L+$ÂX×{?L%nRj%0?L+$ÂX×}?ïé†HG£?}_¦µª V?fy€·¸]?}_¦µª U?ïÂZt曖?|‰ÀÈŧ—?~ÒŌ²5?|‰ÀÈŧ™?ïÆï©hj
?hõ:àûN¬?|ˆ+KÊùë?hõ:àûN­4FGL J2245.5-1734?ëˆå3Ö©eÀMºõýG¾ÛÀ;Œ8ap]`À<Ô/[7^;@!´oˆÎñ?óÊíêSÆQ?ߙ«¢°™?ä‰ößÅÎ@¦-['Ý•@¸"Æ©r¿ïÿSg†!?ïô…¾Eu€¿çÃÉîËû?ÈíPÐÒëË¿ÏÄãIeú†¿ïöºÂM¬AGNbcuNVSS J224531-173357?ïç'£V~?g¿"5H2Ä?hØ\ꩁR?g¿"5H2Ã?ïð'v
?{¤èÃkÑE?_±ùùî'?{¤èÃkÑD?ïWïè·"¿?¤¿w?•é¨&?¤¿v?ïÓfkɖå?p%ábŒ,ó?vLÊ4Æ?p%ábŒ,ô4FGL J2245.9+1544¿áFùF— >ÀBµ‡aˆ±À9ȺÅ­À<£Ä•Æ¦@ 8`Á¥?þ^ŠÏÒ;?ºÎ¬ l?³[;ùç?ôõ]ʶr@
ÌÕHq]æ?îZÌiÐ~2¿çsø :G¥¿Øýç!¿Ü/›¤
᰿ᆚï/:¿Þ!ƒkáAGNbll1FGL J2246.3+154987GB 224338.7+152914?ïþ†ÔSYª?&®ÊèŒ?''ºÊeU?&®Êé?ïþËÕ˜?A!¢6|[?&óB®¦v¡?A!¢6|A?ï÷/j"¬Â?^o»`ïÅ?Q¡*ö¦|‰?^o»`ïñ?ïóÞøx"?EŠý`B¹®?XB÷Ë
?EŠý`B¹›4FGL J2246.7-5207¿ÔPW<ÕH[ÀKê¶â—À:ï/éÁÐÀ<E³Æl@!­#>ô\‰?úƍ«?Å<)¦íj&?³]&¡ª_:?ïÊi²KA@˜»ûÄ1¿ïÿÒ†ëA?ïmMá4c?é°Sº'7¦¿ÀãÛ\1¯%¿âñÝ}t¿¡^ÿÝp^AGNbcu3FGL J2246.7-5205RBS 1895?ïÿ¾9¦n&>÷é‰á.´æ?q–dv¼†>÷é‰á.¶u?ïþ'ËÂ#?EÞ*™DR?/‡ÓCÝՉ?EÞ*™DE?ïóü•?bsà d?XâÅþÓÊ?bsà d?ïû8‹¨q¾?;9<›ê?CÑ^9?;9<›Á4FGL J2247.4-0001?á‹9́Ï<ÀHÞí¢/jQÀ9ÍÊ¢P!À<õ¦	ê@aóA€¨Ý?ÿÖxG9zu?¼¬†hÍ?±©`­Ç?ô=Òä>š@Wëî%7¿êÿ‹ /}¿µ~#qt6‰¿ä‰!S6ß¿Öký¼ug¿ãË=€"¿åv˜B"ÐAGNbll3FGL J2247.2-0004PKS 2244-002?ïù[Ï5Í)?G¸‰"÷M«?JÃ(Ë\æ?G¸‰"÷M?ïüñCÂя?Qø"–â‡ä?8uáés}k?Qø"–â‡Þ?ïä-$mB?t¿¸ Ÿ…?kÒےñ¾?t¿¸ Ÿ…?ïÚôO="Ë?bY€Àhùp?r…ØanšJ?bY€Àhùs4FGL J2247.5-3700¿Óà6Œ˜â®ÀO쿱[WÀ;q?ÊjåÀ<É(˜¥}Ó@+LOŽÞ€@›m´Zæ?Ö>‡$L?¼oU£J?àhÄÓTÑ?ü["ìÝ¿äCt^v­Ü¿ê•êMT¿ã1¾kàú¿á
ÀþŠÓ¿ïÿßHÐSj?ïbŒ•AGNfsrqPKS 2244-37?ïüŠnŒ¢?Ajp­Ã´?;¬‹šëêˆ?Ajp­ÃÁ?ïÞ*kìé?ƒ£Ï²'?pêÊu‰‹ó?ƒ£Ï²'?ï{ðGîx°?‰
Ár?æ­?÷0éÕ?‰
Ár?æ¨?ïê+Zm,ô?[má×wS?eÔ¥'Ó?[má×wI4FGL J2247.8+4413?ïb…-0iÀ*'||R`öÀ9ÄÁA® À<iÍ#3â@!-þËøf"?üb»frû ?³,qMB?Œ#nUY_?ڜb6Uýc@hùÔî¿ìäo¶q@µ?ï<›'Á^¿Þ':_w^Ü¿ßîHÝêVv¿Ízƒ~Ы¿ÙlƒKy{AGNbll3FGL J2247.8+4413RGB J2247+442?ïü;ì½½ß?A.¸Wªjç?> š/?A.¸Wªk?ïü}uۉ¬?Yz|ƒÕ?<Q#²›o?Yz|ƒÈ?ïÈ
/»?p$!'E?{ñy{è"Ô?p$!'J?ïäM'15¬?^)k­¤C?k²}ÎÊTb?^)k­¤L4FGL J2248.7-3235?ÔP…±Ý¼†ÀOyI@»±òÀ9í|7‰À<iÆú$ô¬@htbÑ@⩓àß?µŽ]ü4™?£bÓd÷?êBlA@\gç'l¿Ð㔤è,O¿ç$`ãð€¿é†Œa!Øî¿èœl^Íì¿ïÿÿ&¦³?ïï?ôÕ÷AGNfsrq3FGL J2248.6-3235PKS 2245-328?ïÿ£eñY?
Œ gøbå?&ƒ¿©¶U?
Œ gøb'?ïýð:'•?O‹:ÂTo)?0¾+ëSí?O‹:ÂToC?ïàñ~e"H?p2ZšÜ×?ošl¸?p2ZšÜØ?ïþº™<,?ÉÏ/,?$VnŒ=K??ÉÏ/,é4FGL J2248.9+2106?î£ëâ(ŒšÀ@±Å3À:P.ŽˆÄ_À<[6@KAqåK@·ÛnP?³?ÂT¶ø°?´÷îc c?ñhãï(Ah@V0´RØ?ïS³çc¿ßifËæó¿¿ãÊ
æ
³¿à5ŸI[ê¿è¸ê—¸ï¿ïýc¾yåAGNfsrqPKS 2246+208?ïýL;t?3áç	¯?5ž#|_%h?3áç	Ã?ïýäQ¤P¡?PWuä.Ë?0ÝrÝzóQ?PWuä.Ï?ïá͔̆?r.1…<Ìt?nâ3y2lP?r.1…<Ìr?ïõ;Záª?Bò8¢ôà:?U‰ÕJ<«{?Bò8¢ôà/4FGL J2249.4-1300¿ïI²cÝÀMužèóÀ9<äw
}—À:ô؄ô@ OÏë1@ðúÄV܆?¼^z‰³ób¿¡UWv'Ù?ꋾßK@@½àJÙ?íÊt}€^_¿íz	ç	Žõ¿ÅÄyÇÑ¿é4mÙw¿åCå~*¨¿±ó¸žík~AGNbllRBS 1899?ïÖrå±¼ò?"áA"a×ò?tƍ'!†î?"áA"a×ò?ïþ>̋U?Em#µÎ?,Ó7J›?Em#µØ?ëø1"Ö?­±-¨ä?À;«ñì©?­±-¨ä?ïÿÖ"Þâ>ô(5@
>ôîÀŽüù>ô(5@Ã4FGL J2249.7-5944?è]5ÀI§Ž\NµpÀ:ãÝéTÃÀ<µ&o<Ï@"W'
3D@M++ý´Ì?ƆîFD2	¿Ã~'Î?Çåóö@áÐj?¿ïñüÂ2êä?îAw^o¿ãP¸7åŝ~*¨J¿Äs6X¡U¿ïÿG©ýdAGNbcu3FGL J2249.3-5943SUMSS J224938-594421?ïüá
¨ƒ(?<úçt'N‡?8÷'»æљ?<úçt'N`?ïþ_$Й?A½m Y?*
²öoã?A½m K?ïÊì¾Ó?x "mñ?zÿ󉠖›?x "mõ?ïûUÞã¶?9ØwÜßÔC?Cò¨"q(g?9ØwÜßÔ4FGL J2249.9+0452?íeEõèÀGJiߗª¬À;;m"XÀ<‰U>öµÔ@ÔBŒíd@£ÿYçÓ?ÁÉÓގ쿦ÆcÉuw?ãkD´e@¿o`
+Ó?ïÿQº÷k¿àšPCrŠ¿ãkâ§)¥¿è»F'‹ˆ¿àñÈ.Ø[¿††="«»RAGNbcuWISEA J225007.35+045617.3?ïþ¹8#T?#)‹;&Z?$l}ÎJÈa?#)‹;&§?ïýÇé ¸?H-T—X?1À²ú?bè?H-T—Q?ïå‡éM)?p
Ú¨N\$?jx²ñ×µ?p
Ú¨N\+?ïùõºÇØÔ?8Œ;*,?H)àœ±Ñ?8Œ;*4FGL J2250.0-1250¿ï~Dž&0ÖÀM:'£SÀ7`@ÒX'	À:oîÑ"2@ÎmÚÎî@Ìy1D?šw'ç+{a?Á+±I8®@*ç'Jð¿@!¥r6ð¿Å±Œ)™q¿Ò|	°ÛU¿åÁ£¾¶‰"¿äœÂä¾®¿ç€q¿àÖ¿ïÿôA…ÜMAGNbcuPKS 2247-131?íŠÒÙ)z?¹€|%›Mò?³©l6´(?¹€|%›Mò?ï·ÛÓó?¥æÚ*‹º
?'	8àƒ?¥æÚ*‹º?êKÛï4g?°HC½)²?ÆАC/žd?°HC½)²?ï%®'œ0?§"KüB?›J/ϬyÖ?§"KüB4FGL J2250.0+3825¿äÂ|±'À2Ô8ÑØ¥À9uTáä·À;ð/Þí@!dèŒñÀ?ûi¥ë·sŸ?®ôMS?'¡Ö\¡Q?ä?O™›G@
}ÙªUÔs¿ìô±d "?ǔ$9Æ_¿Ûguû.ßç¿Ó5dæ´¿âÒÐ¦¿´¸¨ÓsZAGNbll3FGL J2250.1+3825B3 2247+381?ïþ'î[­?K
m)sn?&Ñ:E/?K
m)rÑ?ïþ1ÌY¬S?G1¼"?­?,ã:e:ÞÅ?G1¼"?—?ï觏s•?tsÃNPó?gXpŒjõÑ?tsÃNPö?ïùÞyòýÈ??š7Œq—?H†4åS??š7Œq—4FGL J2250.4-4206¿Ôð]ïí·ÀN–HƒýP"À:"ë=ÑçÀ<æšÔ,=@ñ¾1""@¨Ú!I%ä?³ö¢3F(ƒ?qJB¤Œ´?À"z~K_z@"`d\?îE ˆ¡#Ò¿ã
AQ®ô¿ãL¦ló"¿à‹,žÄ{Å¿ãb¼ÃjM|¿Óð
H´ÐAGNbll3FGL J2250.3-4206PMN J2250-4206?ïý¼¤µ¼n?)gD-?2ÚR'%?)gD-Ï?ïÿ
ßðŒX?8ޅÅ_T³?Dîu?8ޅÅ_T}?ïöÀÆ­xV?f,h^D{?R~r¥Rw?f,h^Dn?ïþ¥¦ë¿î?³,ØpÐ?%¥'D5K?³,Øp4FGL J2250.4+1748? ?Á¦?ÀB*ù‡?úÂÀ9ÿI¯vz±À;ü3Â¥@pªEä;@HPïܜ?¶×(˜¿ˆ"¿Ã'~Ó?ÅBÔ{lÝÏ@P",P¿ç%=Ì4¿ëË·XÇAs¿â.LC¥q>¿êaÞËÒÒ¿â£Ó¯?¿ïó¬ÐDÑAGNbll3FGL J2250.3+174787GB 224805.0+173330?ïù±DþÊ/?Iɹg<:?I:ì×H?Iɹg<K?ïþ*½0Ô?JÛ¿£rä?.ýT,ò¹?JÛ¿£rÓ?ïfüӛ?‰²…Ès?ó eŒ~?‰²…Èt?ïôž?´ß?Hº"ÿYq?VÃÿ€–A—?Hº"ÿY‡4FGL J2250.7-2806?È#ÇX£HÀO¨×ƒßóñÀ8{cRµ¯zÀ;™kŸ‹K@#ëÀ š@cTÁ"tŸ?¤õç"c'0?¸abEšh÷@ô‹"'Å@­ñâÝûŒ¾>êw¿ÓÜ#…}ƒ¿â¨½¯"˜¿âo–[ ¸¿ç+úŸ˜â¿ç+Kb©îQAGNbll3FGL J2250.7-2806PMN J2250-2806?ïý§"Y*…?,ÝA¦~mn?2ÃÝ6«Ò‡?,ÝA¦~mg?ïø·Ä6Ã?dd~ø¶Šº?Lõ ï$ôÅ?dd~ø¶Š¸?﫬ÒÅ:?ˆ=îzOh?…ËN¼ñ??ˆ=îzOh?ïÿ"}ëÊ?ªDãº? …?Lì'?ªDã¹¥4FGL J2251.2+5550?ï'ñ¨ÛIÀ	MÔº.À:·¶'Τ=À<ž¡@W@´n œ˜'?ø­ä	)tn?Ք#c‡?â5ð²…"ê@z&3pp@"u€4ì?ï·²­fÖ?ïû"€«1¿ã¢à՘Mi¿Ô×DÈ¿éeã>~?÷¿ïÿ
Çhß½AGNbcu87GB 224837.7+553415?ïö‰¹$AÁ?XÒ5«?R썷|}4?XÒ5ªò?ïÎ'kh?ªnáiŸ
ü?xûìJsËó?ªnáiŸ
û?í«ew€—?¢-¤^V?²¤ÔCû"D?¢-¤^W?(#Ìk?~rŠ—ÿSß?Šu÷å?~rŠ—ÿSá4FGL J2251.5-4928?Êõjü™ÀLù¸Që…À9ÂXr‡ÜÙÀ<;€kË*5@ ÛçœÜÅ?û½.äïÙA?´$í ,ì?º—ën£w@QJZ—%K@•#"™Þ?ïØÜx5?ÓÇ3{¨ø¿ÜÌÜÝ;/¿Ñà¤.Èë¿ß
0eMŒ¦¿äâO §)ûAGNbll3FGL J2251.5-4928SUMSS J225128-492912?ïþÔÿ'UÍ? )Y`ܑÇ?"°
Š£5á? )Y`ܑ,?ïý6¸dó?SÉâ˜jkÃ?6Kò<Ø^î?SÉâ˜jkË?ïâQ´Xª??qwÒüì?m®K§UÀ›?qwÒüî?ïý6áÙÓö?'¸—-Øø?6Hñ1`LÅ?'¸—-Ø	/4FGL J2251.7-3208¿âÏT@›ÀOͳÐ|"¶À;6ªw7oÀ<­[.ú¿N@!V\îm†k?üy0ˆ^ó?ÆÔÏ»¼Ë?g"õƒá\¸?ŠÎ¥rž`±@Sõ.jÌ}?ïQ8×·âZ¿ë©Åá¡A¿Ôìò»ÈC¿àUçÈѕ‰¿æ¶b!Z?àU¹pޏAGNbcu1RXS J225146.9-320614?ïþº€
&?Gº´Ål?$Xÿ-§ï?Gº´Ål?ïýé5˜¬?GDÙìŠI¥?0¶S:Ÿû¨?GDÙìŠI‰?ïîXp§6?sRl^RN?aþ§XÊ>?sRl^RE?ïùü`›æ?<##ënS?Hî}bw?<##ën?4FGL J2252.0+4031?ä'óŸè[À0ã"[tšÝÀ9>Ëò²9¤À<	z‡…›@À'Ÿ:'@Ñ"2w?¯¨Ž¡ebR?¤9¯¤A?ôü…×Dö@	\'»Ô¬ë?ÒÞ&[´[½¿ÓSˆþ–É[¿á–¥ÞÌS«¿Ü|—UG¿â§ýª»*
¿â¡·ªü˜lAGNbll3FGL J2251.9+4031MG4 J225201+4030?ïûø{KŸÓ?4ä苚'¢?@р±z?4ä苚'¹?ïü"ä¢Ö?X´bd‰W<?;XÚï!Y?X´bd‰W:?ïõ;)£L&?Z¤ÄíA"?U‰¬¹g²ò?Z¤ÄíAl?ïÜ=¢V—ù?]JYÉØ?qá.Ô´O?]JYÉÓ4FGL J2252.6+1245¿˜Ic'¿×ÊÀDf¸w«À;<Ÿ1‰À<œ׊•ñ@ lià™]?þúEዠ³?Ê£âëE?½g³¶Ñ?ò"ßq?@@Î*oë¿ïÿýFKê?ïû×ómK?äÜ7£~ö¿çOHÿ΂¿â•Oçžà?µüé=ÝÜAGNbll2MASS J22523220+1245109?ïþúÚåi?0Rºêï¸?. RQ©aš?0RºêïŠ?ïûIp&"¿?eZCëë"?BÚ?gtþº?eZCëë—?﵍f¬1À?ƒšŸ?^Q'?'œ¦TóÎ?ƒšŸ?^Q—?ïÐV´³i?k¹ÝÖy6?wöÔ¥¦JP?k¹ÝÖy74FGL J2253.2-1232¿º•ø5øҏÀM]Ñ_ÄÖÀ9ß=ÍÀè"À;À®J*Æ@*ߊ¿¥@ÚøßzN?Ô€"ØA?á©é"mé@›ç¢;(Ë@à{/Ì ¿á×xø9b¿æ=¸È3
¿å¢Z¾ž
¿ìÿ atd+¿ãHY€NïÒ¿ÐFPܼYAGNbcu3FGL J2253.1-1237TXS 2250-127?ï†}›€º?'ÍaBôˆ)?Ž`™8ŸÑ€?'ÍaBôˆ)?ïüçþ¾ä?RR5}‹q?8À
àßù?RR5}‹u?êûߺ`¡?­ö Û˼v?ā¢}"?­ö Û˼x?ïâåé:D[?aڝFΣ?mÅ»¥°?aڝFΤ4FGL J2253.3+3233¿°3;£âÛXÀ8	"‰a=À;-Ëë%À<fÙþ
·y@ 4ÓÇ=@o³·RE?ƒìÁ´À¼¿€Ã@ö¯
8?¹!˜¿/@g‡ÒœÅs?ïù]¹ïzw¿ßmµ»
\µ¿à²ž­›¯¿èòÂ?U*¿àq¹KÈ˿ے¤²ÒOÄAGNbcuCRATES J225312+323615?ïú\Ä
Ýl?E«U³^H?FŒïԊP¿?E«U³^C?ïþ°¥Že/?H=¨å=Ä?$õ§­:?H=¨å=Ÿ?ïÁÍ'â?}«­âK…?l}õÝ?}«­âK?ïõ•Ðï´?A¡lËš»?TÞÔ^ ˜1?A¡lËšÝ4FGL J2253.7+1405¿ïZ­ÿ,œÀCîWûi˜JÀ:Îb«ÆÂÈÀ<v²¹%P@ ¥‡4è&?þLhĸ*?ÇläDb°y?À|êŒP[?õºÂùå3Ì@—dÌÞ?'?îϾB'¿íè¡^ßßN¿¸\2ZñQ¿âHMv«X¿Ý&-;L‡B¿ÙvÞ¸1µAGNbll3FGL J2254.0+1403NVSS J225354+140439?ïÿëÂûA?"}ÜU¯U?¢‡ —ßÀ?"}ÜU¯<?ïþA'™¾?Cmˆë2lª?+ææd†t?Cmˆë2l¨?ïöò)š¦k?]…Ÿ¿
Ž	?R¬Ê³,"?]…Ÿ¿
ù?ïóDE5?Hú8/و"?Ywuӕú˜?Hú8/و'4FGL J2253.9+1609¿Ñehu!:ÀC©~+VÀ4ºaŸWH¼À:›²xŽ@ˇįó@K̼ܔÁ?|gÈ_V‡?¹¬‹cË×Y@C‡~|â@%ᖏùÞ¿Ìú'WÛß¿â3ÂÚۃI¿æÎÇxÏõ¿æÊֈ7q†¿ëa#0†°‰¿ìVB+ÐAGNFSRQ3FGL J2254.0+16083C 454.3?휨'Ë´ü?³zmß)@w?³»q¢X%?³zmß)@w?Ð9Ì'°Ãß?Ù·ƒz›f?çãì'ž?Ù·ƒz›f?ê³ÜÅ<?¶?®æ2uۀs?Å0Œë(?®æ2uۀs>w¡îU&>®óú2¢"©?ïÿÿм#T>®óú2¢"¬4FGL J2254.2+4305?èJ€ÞìÕÀ-'L¾´À:‹"XÖÀ<Áh¼P@ª>0'D@^e'
?»öùŠp¿p7}¡"°?­xŽÃ8	Ã?â%ébs¿áò_-¿åcŽDÑÁ(¿éÿ½Ñb^¿âíŒM€¼¿ïûS]u&?ï¸d*LåAGNbcu3FGL J2254.6+4253B3 2251+428?ïË!"'xn?­"çKš!?zon¶ÃÈ­?­"çKš!?íE'
.Â}?Ä*Ê"±?µÖÇ®‰ì?Ä*Ê"°?£MÇ? ~¸ÔÔ5õ?¯ÆË#…? ~¸ÔÔ5ô?êu»!@‹?µÌ†ªñÕÀ?Æ)ózý×?µÌ†ªñÕÁ4FGL J2254.8-2725?í²¦51[ôÀP	ÿÖ"îÀ:D¶4‹À<,ü<& ü@ ×0;Üúí?ÿò‹ÿH?ÀœÒ^18²?:燎)N?ÐɒZ¶@·{ý+?éý+4¾y¿çª|?ì¿à»²}ì¿ÜP'¤_›F¿â"?_'`¿ÅÑûÆ_uAGNbllNVSS J225453-272509?ïþÝøûë?•œwÎQÐ?" A4.?•œwÎQ›?ïþålÆæT?>Ý
÷:Ã?!©3'š­Ò?>Ý
÷:Þ?ïúgçø|O?PxÝw?F``ÃÅ?PxÝX?ïþì0S¥Á?%¼(øF?!<úÅ£þÛ?%¼(ø4FGL J2255.2+2411¿ë·MYòf4À?ˆ;`(^ÄÀ93´±M†À<IF"@n[4Ùü`@Ûª€qªg?¨àA¸uí¿Uäa`d'?±¯Û @Ê! c¸6¿áþ3a¬Bi¿áNË?.¿â<8*ù¿áŸà¥Ç¥F¿àßÕó¼ûž¿à&JLTliAGNbll3FGL J2255.1+2411MG3 J225517+2409?ïû¼è F?8°'¹J	?A]~çÁÕ?8°'¹J	!?ïþ°"&­Ô?@Ç
-?$ýݕ"²G?@Ç
??ïëËV|+¸?o†èâM?d4©ƒÔGá?o†èâM)?ïø㠚Þk?Aad¥½Ü&?Lq}"†V°?Aad¥½Ü*4FGL J2256.0-2740?ï«Ék¿PÀPýŸÓo~À9<çƒ1xHÀ;Uù†i;-@åBÕ<²ä@¡…÷%f?´f~«<ë?'Ÿ˜6B1S?ÚÔ֜?@	ðÖ. Qo¿ÝŒZ@é)O¿éÃÌÞj"¿êˆì9ò¿êŸ<¦y{í¿ïÿtN†v?ÇÙ府mAGNfsrqPKS 2253-278?ïÿ¯ç`Ž??
b`¶vF?'Üpp?
b`¶uú?ïó­ÁªP?s«,í]td?X¤|«^Þ7?s«,í]te?ïNå;Á?Ô	±a?–#\ý؇é?Ô	±^?ïøìzåa^?B¢Dô/[ø?LNjzƒ•?B¢Dô/[ð4FGL J2256.4-7119?ã*®wÒÚÀE~p\‰mÒÀ;~à^zÛÀ<âòŒyöf@""'y´¤?ó§®ë:v?ÓmJ[BñÂ?Ûpmü1ê3@ ÀŸ—à\@õƒÈ!{?ïû¼PíX¿æá¨&$W¿ïÿïXz?ïÿÝ/ñ_S¿ÖA9†3‹H¿Åüº¦.¨_AGNbcuPMN J2256-7115?ïúílŠiþ?L։">cÎ?DJMÖX	¡?L։">cß?ïíÆÑK?†Elaˆ^?b9.´pæj?†Elaˆ^?ïhì"f²Ó?Œ‰hG÷œ€?'âm")¥©?Œ‰hG÷œƒ?ïí:i ó?b:LÞTK?bÅð–_ž?b:LÞTK4FGL J2256.6-2011¿è¬'ð·ñ ÀOr" ٔ[À9cÑû	öúÀ<1¾Ûrþ@Ìâ'q	@À5¤'?¬˜ßàOáj?šgà9B?íñg™T@D
ájÿà,RÚš¿ßECÁu֜¿ãy î?
¿ÜEíhMÇ¿æƒ_—±¿äiM š)aAGNbll3FGL J2256.7-2011PKS 2254-204?ïäh68ú?bî-¬T%?k—ÉúÇ?bî-¬T&?ïÚàƒu¨?› ‹ü?r¾Er,¸?› ‹û?ïž{ÎëOï?†sc/WJL?ˆaE,^?†sc/WJO?ï¨Dðh?wO—Ê'?…üîÃåü{?wO—Ê"4FGL J2256.7+1307¿ïY ú
‰ŽÀDˆŠÅÁ@À;~d^NÀ<5·qñµ@ S‡QŸ¯?þ+£!h0?ÐKÍ=µî?Á•Æü(Z?ò-žž¼J@žx±A«ò¿ÞÁÍ_™Ã‹¿ÎÀ¸Azsº¿Ø«hC`Qú¿Üö)RáP¿àVÎþÖ4U¿ïÿóÀ¬ƒAGNbllNVSS J225624+130541?ïþè pÑ7?d<ˆ%†?!uøòìŒ%?d<ˆ%~J?ïýÁx—ñÎ?M2	ÌuZA?1ô;@q‡ð?M2	ÌuZE?ïå~}ÞbU?o gÅÞK?j'!ªo?o gÅÞK?ïîø¼U\?PÂôŠrRM?aðCª£¼?PÂôŠrR?4FGL J2257.5+0748?ÜS¦‡˜(ÏÀF¿ŒâÑñÐÀ:֟vRl´À<n¡¾+IZ@X>A¯!ì@'ìCŠ™L?Я¢šÛ¹?¾1ì'9ÿ?æÕL}‡\@«QȽ/¿ç8"Üû¿çwk§^¿ÓàŽ€`ãp¿ç͑¸ú‡ñ¿ïû5`4>?¿¦Þüz9'AGNbllOY 91?ïúøP©P]?G/Äu¢ö?D½Z¾ˆ²?G/Äu£?ïø›TZ?dmâŽu©£?M'­ú—Æó?dmâŽu©š?ïXØOqãz?‡v©¶ÿm?"äöÐÂ?‡v©¶ÿk?ïïšÏt¿·?P†{:{Ðg?`e0‹@H?P†{:{Ðn4FGL J2258.1-2759?æçüý,6ÀP;0"'À8=RpæÀ;Sß'Bd)@ ÔûðPà@L…0aÈ?¡€Å?î?ÉVEÜÙ	q@#–žš@¼à€ø¿µ¾!Á¿ÛFËÿ€¿åM1:Æ¥¿è(bTˆîQ¿ëOý¤-f¿í
òl™†NAGNfsrq3FGL J2258.0-2759PKS 2255-282?é3¾ }€?"ˇ½Í?Ë£1~	þ?"ˇ½Í?ïà'}UJè?'¬PãhÚ?om'ªµë?'¬PãhÛ?æ'Ûç!þ?²í))bþ¦?ÒÚH1½ø?²í))bþ¦?ïÅVi†t½?vɘO­èì?}TË<Å¡C?vɘO­èï4FGL J2258.3-3643¿æ1ÑuñXÓÀP*0U2aÀ:–…`ýpÚÀ<¥šàÁvW@V¯ÂÐʈ@š"ù$D?ÀlrYŽ¼œ?£tå㧸I?ãm­¸4T@	9Yèԕ¿ï`ƒ-FŠ(?ïòI~N9Ÿ¿Ü)ªu[Í¿éŸKT'(Œ?ª›ÈüfK¿èW'[åYAGNbll3FGL J2258.2-3645MRSS 406-025483?ïý™×ƒ?1AyĽ?31G×Óçw?1AyÄÆ?ïþƒØîR/?ElVm·?'ÂqÝ"?ElVmœ?ï¿7Càäð?~¸ÒÜ^?€2/ÆÄ??~¸ÒÜY?ïþ-LüŸ?%_¨y¾ø³?-+06‹õ?%_¨y¾ø]4FGL J2258.4-5524¿ÜçCÛÙB§ÀK;Oag#À:aƒ3%Ç:À<¯
@Ë¢*@ya¸âÔ@(a´Oþ?²ÓÁž‡Á¿¬§i¢Q?úPŒû%¥¬?ÿÐÈLŠr4?ÄÍÀ"!¿çÓ²ßæ¯ø¿ãÔ%¼R+F¿à"ØÅ0 ¿Û]:É)ª¿æAž¥AGNbll3FGL J2258.3-5526PMN J2258-5526?ïÑì2ØÖ¬?sõw(t›ó?w	擔ª/?sõw(t›ð?ïîƒ
lż?u¨?¡Û?a|ò":Cz?u¨?¡Û›?謹Q?"¾ÁºËyÂ?…P+¼þ¹Ë?"¾ÁºËyÁ?ïÿMØ
'?sù!²þ!?ˆ€,‰ý_b?sù!²þ4FGL J2258.5-8247?ä̀]fÀ@¶ YžØÀ9Г¯tÍ1À<4‹ƒVa6@*wB+ɇ@¥ ¶Xí?»]7ÄB?ç-@÷Ý@A¶Ô=—@:«C:<g¿à.'à¿ÙÈõ<WŸ#¿Ú!(¤c÷÷¿Ý{ñ½òêC¿éEÚÍa¿ãdeጢAGNbcu3FGL J2258.1-8248PMN J2258-8246?ïÌx8&b?|I[Nœ?yÃãìη~?|I[Nš?ïûn¸/?[FÞ¶¨Hh?C«ÆEH[?[FÞ¶¨H\?ïóC·ÌU?—=&™N
é?!—‰ui?—=&™N
ê?ï½ïoàeŒ?oGUé¸?€"$æ,?oGUéµ4FGL J2259.7-3549?íõ"Üj7ÀP05~gÀ:zj]këáÀ<•ýÉÄÛ@ì&.6Ÿ@ewmÏ?»¤ðñ4‹¿"ž/aê›?ØñOƒJø¢@žëq}›·?—¿¸€ÿ2¿¿èWï«&\¿æ>´`šI˜¿×wR|¤–M¿í þG™ſĒ©ei'>AGNfsrq3FGL J2300.1-3547NVSS J225941-354846?ïé .µ"?d9–=…Ë?foßÑJm.?d9–=…Î?ïüi3+ºt?UT¯*O2?<¶f¢,Vw?UT¯*O1?ïÊÖò½ù?jw™a?z"†·¡á?jw™^?ï÷µ§Òt?AÑe2þb?P"ü°[Û?AÑe2þW4FGL J2259.8-1552?íZHT88|ÀNå‡?úÁÓÀ9ùqÆùgÀ<`9»°è@7/
.­@DJ9ßõž?º+œk[?ºÿ"JOY…@µ­é¿@b?Š.˜¿Ò¿žÁ÷‡¿ÜÂn$ïß¿ãbåþL À¿à®°³ ¬¿äŒñ_Ô&¿é¨eå7&ÞAGNbcu3FGL J2259.9-1553GALEXASC J225957.26-155332.5?ïýú¡úóB?'CêîP˜‰?0*ð(eõ?'CêîP˜z?ïýÕ@V|?LãÁÚ
?1WýýLw?LãÁÚñ?ïìú¯:?hz˂¼ž?cPÅàü!?hz˂¼Ÿ?ïûó \—?1{á«b›B?@3§u?1{á«b›Z4FGL J2300.1+4053?è¡‹£"ªÀ1=³(é-À;4½çXÀ<œIwBV½@":QŠŒ5ƒ?÷˜ƒ$"?Ó¶, ð;?Ñ5@Ԇ€?ú…dÃÎ÷I@õ˙Fª?ïpŽ• ¿ïúS] ;?íÒ ¶ÄLÌ¿¸úÕ^@Ó¿Ð9*ƒŒ<¿Ù?͚'AGNbll3FGL J2300.0+4053NVSS J230012+405224?ïý³‡næû?.ça¸€?2cĈÈ!Ö?.ça¸v?ïýc$FE?QD3¡ÑÂÎ?4æÝÍ×Ó?QD3¡ÑÂÒ?ïÝx¨?±–?r¹j| d?qC«à'4Ì?r¹j| j?ïí¢+Zç?Ymøhž_´?b]Ôæ¥0?Ymøhž_¬4FGL J2300.3+3136¿ë4´e˜À9'ê>xâÀ9'üaåÎÀ;øV"ŒÂ@d?3F©]?ûÀ§$œ—?´(Ùþc´?Ãï$eü¸@cÈ}²³F@Qä&?ïæªY~?×êdbU4»¿Ôòñ#Ä*g¿Øj'ò"È¿áæïÃqÚ8¿èŠ.A±ÑAGNbll3FGL J2300.3+3136NVSS J230022+313703?éÅZ"?ÂÙ`ˆàZ?˸ê•íù¿?ÂÙ`ˆàZ?âчãß?Õû¦
{ç?Ú\ð8AËè?Õû¦
{ç?ê®#×{~?­ŸÚñÎ8¡?ÅGp¢ê?­ŸÚñÎ8¡?⎩bµ(á?³Zn¢$`?Úâ­:•®>?³Zn¢$`4FGL J2300.7-2645¿å ³õÄðÀPWæšÔ,=À:ݲ"ý[
À<{k%@áöfÏÿ@i=¾§p?ØOsûÐE}?ÙNäH•@:ßdš@Næ¤g¢¿Ü÷K%˜?ý?ìԝ¡;#˜¿â~\&qƒÑ¿ä‡ä€G¸ü¿ïý~E€<ѿ䈴€ÈAGNfsrqPKS 2257-270?ïñ¡±Z®u?d<—ô̐?\¼J£?d<—ô̍?ïý"´½H?Iv^'†x?3ZZ¿Qù?Iv^'†…?‡Ûø?–^'jET?§u'O@t?–^'jEV?ïïc×dÚ¾?T±G,/ò?`œ(›%B?T±G,/ò
4FGL J2300.8-0736¿³ïf2¦ÀLªt)ˆ<À;1²åšùìÀ<¢f®ŠÂf@ ÔÏj5þÀ?ÿ:o¸¿ß?Ã÷¤;Þþ¿§öO¨ó?äëûѝ&?û²{诿ì,¸Å®ËZ?'¿FÚãn'¿ã®ÊM–‹È¿ÖÛt/|ÅM¿åÛ;à€Þ¸?Å£3÷(kAGNbcu2MASS J23005469-0735438?ïý™HBS=?.1ê	E…?35½íf"Â?.1ê	EÂ?ïîöÅۙÄ?wbò¡çÖ_?a	:$f<'?wbò¡çÖ]?ïð­Q†Ò?cҝ–ށ?^¥\óÞ[x?cҝ–ށ%?ïÙî.'ò?dæ(Lâ.?sèý·O?dæ(Lâ.—4FGL J2300.9+7108?Þ)¾í¨@$XNaŒâÒÀ;B* dúVÀ<¡'~Ê
{@ íœøž·¼@g£Àd¾?Ö2%™È"?ÝMŸ$óÕO@0K!f'@F2"QÜ¿ï²BÝË!Ò?æ÷,Êx?ïÿ×ñÃý¿Ú°ïáú±b¿ê\Ö/Læ¿ÚgC›‹6TAGNbcu87GB 225907.3+705409?싗Ä;…Ž?¸'o½þ ?»£AÞ#ӌ?¸'o½þ!?í°û¿$¸?Áƒøaû7?²x"ߺ@?Áƒøaû7?êò«Æ¿Æº?¬û|^±Ä?Ä5Påå?¬û|^±Ä?é¯ѶH?¶÷zÁë…?ËÁCì¹&ä?¶÷zÁë…4FGL J2301.0-0158¿ì¡É_·BÀJÁ—¢H"ÄÀ9KþmuNÀ<͆00I@	('Ö¶@ˆ+輜?°ðZE›À?»{u·O¸@S;wG@¯ga8)¿¿8¦³³v¿á垪Ðy¿æ½}h5ž¿æ†yKD!¿éïj¼6|"¿ïÿîbHÊtAGNfsrqPKS B2258-022?ïþ´LqèÉ?qLCקë?$»8ásx4?qLCקà?ïý)*ièß?MCͺÀ ?6¶¬°¸ýÔ?MCͺÀ?ï¶ÃËœË?|3¤õ%D(?'O
>˜Íx?|3¤õ%D%?ïÿö]eA?¥ú¦PS?h¦°?¥ú¦P4FGL J2302.8-1841¿Ñÿ‡•ýöÀO×L`RPÀ:»¸/†ÖHÀ<¡Èê¿üÛ@ªòêí¿@ä"]?v8?ƶgZ­³?­1÷㕪æ?åÌÙAÐ/@]tWjÊú?ì!ÙzZ9¿ä¿'Bd(Ÿ¿àüö•óò¬¿áï;â"D¿æZUÖ¿ïÿo˜AGNrdgPKS 2300-18?ïõÉåÜ¿X?LG¼w×I?Tl4FRí?LG¼w×<?ïú…‡i¢/?\(,‡ƒ?EéâYw@c?\(,‡˜?ïÞ_­ãe%?rDÄÝ1Àï?pÐ)Ml¥?rDÄÝ1Àæ?ïÞs¼ðý€?Zc-¤üé?pÆ!‡?÷?Zc-¤üæ4FGL J2304.3+0618?ì•÷`¯ÀGÙmã2iàÀ:¢iÿxÄÀ<`FS¡gÄ@¾
0•5@úxCÞ|"?Ï0Æ[ïj?ÍGÇêºÉj?øc×ZÅHt@
å+|…Œœ?ïþ~ÀÐ?H¿áî÷. &|¿è™¢¨áá¿æð(A<¶?¿ïÿ¿h`;ª?ïZZ¿i6ûAGNbcuPKS 2301+060?ïÿ>j8Ü?N(O'À'?2¸ä~W?N(O'Àø?ïüjUJ€?S¦±7{œ±?<­WE«ôÁ?S¦±7{œ·?ïY"I^¹g?‰ËòœV6z?"Û¶Ô(Ó(?‰ËòœV6~?ïõE»Ãl?Iï0é?Utˆyï)5?Iï14FGL J2304.6+3704?ïirç8¬À5¤]AúvÀ9"n"2QŒÀ<XÓÖ¬@ TÐó"?ýpoiDg8?±—÷-š?}ÅmáC¢"?Íè¤CÁ Ê@
/¬G¿»¦æÿ(¿Ûl¢ Sr¿åï¤"^¤¦¿ÍEþâô¿ÔÑ{ˆ6šÇ¿Ýá/ÅÀiAGNbll3FGL J2304.6+37041RXS J230437.1+370506?ïÿm²ßÉ ?¦ù¹›>?I¤Ûö ?¦ù¹›Y?ïþ¨mk,h?A퇳ží?%y)M9Žx?A퇳žè?ïõãºaÏè?Zh¥LŽ?T8‹<`-Í?Zh¥Lã?ïÿ46?ååޅÜ?yp™c?ååކN4FGL J2306.6-1105¿ÕÃÊNè°>ÀNMêhìSÀ;+š8ûÊÀ<¢RÃò2¸@ü%4ÂÕR@éĤà¹?Âìv¶?Ž¿œ«ÒèUûp?Ü}Y\'¨?þdÐTÖ×?îI±Y¤·?æ*¿ëò¸ࢿÙÅ» 'è¿ÈO8·×rB¿æ®"2Q‹äAGNbllRBS 1943?ïîŸ	cit?\fÛº¯ìF?a`öœ–Œ?\fÛº¯ìU?ïóY³âD?zð´ûˆ?YL˜;wõc?zð´ûˆ?ï×@MÃY?sœe3Jv?t_ÙqÓh?sœe3J{?ï᝺}8?að_mñÔ?nbàE'Ⱦ?að_mñÌ4FGL J2307.4-1206¿ï2ªúÆ@²ÀN°µˆãhñÀ;JÅø5À<«¤¸²@ Î
ŽÞՎ?ÿCýrr
?ÅGQù#¿'ŒÛñH?ÐõêÓH@Š‡À©(?퓿e=W?áÅÂíOú¿â¦ìq­Â¿ïÿêf:Ç|?ïÿž{€©ß¿á¨Ðº%*AGNbll3FGL J2307.4-12081RXS J230722.5-120520?ïþeÛdÙí?0ow?j¦B?)¢I²a:8?0ow?j¦b?ïþ$-@þ†?IسQzÒ?-½+ð¦ß?IسQzÔ?êä#§?‡}¨= ´@?‰›EF÷?‡}¨= ´=?ïþŸ1ž ?&VÁցÔ|?&榞?&VÁցԴ4FGL J2307.6+1451?är#ónËÀD…Å3À:!ó¥~ª*À<*¬3Ð%@AÎ\
m?ÿä̝Òä>?Ä;9ýQÏÖ?Ì
ɲ'@¬Á^ڀê@G¾Šß¿çëi~J‰¿ç¡ŸÒò¿Ù:€™îS/¿âßN_¤¿ä:aûš°¿é{bŸÝVAGNbll3FGL J2307.7+1449MG1 J230734+1449?ïðÙÑãÉ?_ö³Lèv:?^L\9üo3?_ö³LèvB?ïþ2¿¡&?D»SîñF?,ßôí³ò?D»SîñT?îÏjoù?™Aǘ¹?£é^‰?™Aǘ¹?ïý÷ažŸ?#<¬£¾1?0Dóá\?#<¬£¾X4FGL J2308.9+1111?Çý›HUÓ ÀF)Q֌i/À:¥àªÐ"ÃÀ<uý'w>%@öª'».@(…ZGt3?ȎpÜ.1?Ò«3À ìà@3Äz@a¦ˆ›p¿ïÿúŒ—Ó?ïÿÄ}îB¿á¸rØd°"¿åVõ°å_¿ìnç©Çå¿°ûUvT4AGNbcuMG1 J230850+1112?ïàú{+žJ?w/ØË·?o"Ôa¶Œ?w/Ø˼?ïð_ D~?Žd²åNÖÆ?_@¿w̞?Žd²åNÖÈ?ì†ÉûJx¨?¤ÖbèÆw+?»É°%¬:º?¤ÖbèÆw+?ï²YnVö?vhÍÁeÇ?ƒi¤jB~½?vhÍÁeÇ~4FGL J2309.7-3632¿ïP¶)'AºÀP¡¸€®À:&AؤmÀ<rÐîš}@Í;­*E#@,™»þHp?´ '§7¿•ye»Vê?áìi ,°¸@¿­QÝBf?ïþÖj€˜¿ä\º:#è¿à5ŽÂ¦^¿Úr¼€Nnù¿â'—|ˆç›¿ÖàÀ48ñAGNbcu3FGL J2309.6-3633WISEA J230940.84-363248.7?ïú$.\á?Dûå: ?GoëFŒtà?Dûå:®?ïúgëO¼T?aHSeË£?F`RÁ­O?aHSe˧?ïá¢cðÌø?t·ô-¸?n]œ3[?t·ô-¶?ïá"ÁÞ?YÓåÄæ?nã{>!ô#?YÓåÄä4FGL J2311.0+0205¿æ"Æ`×ÿ&ÀJºÇË)À9n‹îNÀ<*ÀY!†@O²(؇@Üðû?±'®*?¸UW༘Í@HçÖyõ@'~k)¿å•XA_›Ç¿Ê1V?Qпâ*È˶LX¿çy]ä☿ߺ?<¿ë…Ð>qT×AGNbll3FGL J2311.0+0204NVSS J231101+020504?ïýã<I°ž?0&!}Ò?0æ²{z?0&!}Á?ïý0£KÒñ?Q`âM!éô?6zå¡hw÷?Q`âM!éè?ïs¦
E?ŒçR‰ý·?'‹>­÷Oä?ŒçR‰ý¸?ïÿ5â)ƒ?5G"yH?]ãºÏÜP?5G"y=4FGL J2311.0+3425?ïǦ*L"À8煵·À7Òv pMpÀ;žq—òÐm@ò E>y@ëDå^³?˜lð÷¬ýØ?¸YaL1‡@nƒ
áÛ@l7ñ³áï¿´º`
±Ä^¿àÈÊ^³i¤¿å˜9²©5¿å&[^u6¿ë¡ê Ðâ¿èç=@Ó.çAGNFSRQ3FGL J2311.0+3425B2 2308+34?ïôf71î?W!ÅY}óë?W3בœ%?W!ÅY}óà?ïñÎ¸i?t…6Òàº?\Äb-áæ?t…6Òàº?ïB­µe?"Ê)aYÞH?—¼JISh?"Ê)aYÞI?ïýüÚ"¢?$# «ž?0/ƒZðt?$# «i4FGL J2311.7+2604¿äÿ¢¥ŠÀ? ˜€"åÖÀ:)Ö¢8¤ŒÀ<Sæ
ær@®¦xÓ{@!§ýàk?¼m<ïI¤d?©ÍáʵÆK?뙟}^P@•\Tê"?펄'¡WÔ¿áPž1Ú¿åà iA¿åé¯nî¿ä¯^'AcM¿ïë»MlšAGNbcuMG3 J231144+2604?ïþ[(:Çj?!"Äí—?*M|S‰mù?!"Äí—+?ïþ<:Ǽ–?MX¡Uê?,<S"6¯R?MX¡Uò?ïê\ù®¦ß?jWϳ|;?e£QY"[?jWϳ|;?ïþr×*)¢?Ðy·Ž ¹?(ҍ]eøÇ?Ðy·Ž 4FGL J2311.8+4541?°¸Èx&îžÀ+}´í²öbÀ:ˆþ{À<4å†×õö@»›¢|@|ôètÉ?Çï­7OË?ß"š‰®•?÷ï~Þ,p¡@×mŠNÎ?ؑÃâB׿âÈñ EØ¿êI
Z[–)¿á1‰Ÿü_7¿ïÿø]Ê5™?íÕx™]4AGNfsrqMG4 J231144+4543?ï Ì#€1?'kggã?‡þÌ÷ó×?'kggã?ïÏYC4˜?š ¶ç²Æ?xS^uå´±?š ¶ç²Ç?ï'Õ/9?"~éïh'ø?ž;Z?"~éïh'ö?ï¯5ïý?têè.,ì?"2¿D:À@?têè.,ê4FGL J2312.5+7241¿ê"T¢™¶˜@&xaՈÀ:Áñx}ÀÀ<4^[Õê@Uyqk'@{¹Fk?Ȗ³á‰9?פõ'Î{ù@¶l£—I]@¤Ge_M?ïÿï9_J¿ÙÃSÜöæ|¿â§§^~:™¿æ……t¿éþ	ù~¿ïüÓ$Õ¢^AGNbcuCRATES J2312+7241?ï¤yåžìÜ?¯kÜë72f?†á†˜DÉ?¯kÜë72f?ïã	bm´®?†u¬zW!q?lö'KP©?†u¬zW!s?ëKvŒÇ–`?«e@Ií
6?ÂÒ%Ìᦁ?«e@Ií
7?·}?t΋Þ"?ŒÙ;ÛÒ ¤?t΋Þ—4FGL J2313.4-6922?æÍ¥ˆnãÀF²SCsóÀ;Ÿ]ZN*/À<ë{o'V@"³u†iæù?÷Ϧ©?Δm_ÔÑÔ?ÍG,å;Xœ@>;¤ò@åÃèL°¿íu/¢/k¿ÖB²A±%Q?ïü÷"
í?ҁüœÌ¿ååwÞ³Õ?ÓPúïIúAGNbcu3FGL J2312.9-6923SUMSS J231347-692332?ïÿ
zÞÜ?äÙPç~?P¤$~"£?äÙPç5?ïýۃæ'7?Nopøšd]?1#àËnHì?Nopøšd[?ïÆ»tà˜X?cÕ´
Õ§?|¢E³Ô8?cÕ´
Õ¥?ïûVHK6a?<ˆ1ôÀÔ?B¦ÞÓ&}8?<ˆ1ôÀè4FGL J2313.5+3945¿ìÆ[ž¦m®À3U<¼M#À9³¨eå7'À<!ܘòª­@½sßrl@=ŠT'8T?»òÂ?U*?ęÎØþ´@¨«ÕÜ@@`äƓ¢µ¿ÃÔ¤¯ò¿æl{=ãæD¿é¬MÑD*Ò¿í(~#qt¿àf6`]'¿ðAGNbcu3FGL J2313.1+393587GB 231102.6+393314?ïþ£Ê"ÆÁ?'g:úêè?%Ã]ӓþé?'g:úë?ïýCj%qª?Q<=i?5ä®Ôr®ê?Q<=Z?ï+µPç‹é?âûòÇÒ?š‰Uã'é?âûòÇÒ?ïþJ@úz‰?‡­Ðeq?+[ðXWeó?‡­ÐdR4FGL J2313.9-4501¿¼Ï¢-ãÀOÊìë¯À:R€;$À<FÅA¾q@½UzþÂ@H.D¶é6?¼/©Ýˆ\?"Ö^úiñ"?ÐD4¢Éî÷@dÕcIP¿æ"G!ý¿ã?¾&@Üi¿êù­ ·›¿ëÞµbLü2¿¾"V7$¿ðAGNbcuPKS 2311-452?ïÿM?Áר?V'rÉN?XÅ
þÊ?V'rÉÅ?ïül÷/ß?Y̐ÊŽï?<˜FñY?Y̐ÊŽü?￟F†ä?#ö•;¯?€.^z†ì?#ö•;¶?ïýžhÏÊ?*Í5X}Ž?3¹¯íÓ?*Í5X}R4FGL J2314.0+1445¿êçoD³+€ÀDôsš¿À9¶L¨O?À< >ÏH¨@ ajNÚY?ü¾ú1‰æ?µίP7?¯Ø\"Ó?û½CÂÍoŠ@JÆ!âÔ¿Ø°îŸÛR!?â盺Ü	¿ÞßÑ ïcÑ¿ÙT)McÓ¿ÞþGï¿Ö›;$™<}AGNbll3FGL J2314.0+1443RGB J2313+147?ïïqsnO©?_¤îÔR?`ŽŒ'°Vb?_¤îÔ`?ïù‡Šî8z?b«Ç§­£»?IáÔGe?b«Ç§­£¿?ïÍî[L`?zð§¥ÁZ??yÒxYϒ?zð§¥ÁZH?ïšÄ"ÅcP?v]ù•v—?‰NÚΧ,I?v]ù•v•4FGL J2315.6-5018¿»viPæ¿¥ÀN?Žâ†ruÀ:3"_ôöÀ<zäÎKR@×5›J@N_œGÉÃ?»ÐßoÖk¿B'Â%™?К©#¥K©@=tю'¡¿ëåN¾©ô[¿Òe­ÄHﳿæê~Ž{X¿àµâoÌ@¶¿îÌaË¡ÿ?ÏÁ¡
&I–AGNbll3FGL J2315.7-5018PKS 2312-505?ïû_Ã(â?A—'(ñ›¥?B€ó\wÖÞ?A—'(ñ›³?ïþ•Æõ?@ð㟄Z?&®3ž Æ»?@ð㟄S?ï—øÑ'"?‡¬Ž,¶CÃ?Š˸Ûw²?‡¬Ž,¶CÃ?ïÿ#Eν?=éS,?—]¦(Zù?=éT4FGL J2316.9-5210?Ój`ÐWjÀM­ÝiÓÀ;)û¤P¬ÁÀ<ÐÄe¨Ñ@ T
$Ç	¿?û¡Îl	=–?ÒÑE= ó?¾ùÝ?û\q?çt/è%ç?ÿ©F«
/Y¿æ5à¿ék×3X¿ã¾+Ÿ@!®¿Æßjßÿã@ä̝Òä¿Ú½†þâHµAGNbll3FGL J2316.8-5209SUMSS J231701-521003?ïþÃ,;ÔW?β¾?#Í<BºvŒ?γ-?ïûƒŠÖ=è?a¨ÄUdmË?AñÔ§]e?a¨ÄUdmÌ?ïñtmÞÐx?f=´Ó·F?]$B_ø?f=´Ó·8?ïõ<xÄЭ?GßÒ	*?U‡v^§Ð?GßÒ	4FGL J2317.0+3756¿ëoߣ!¾îÀ5GvĂ{pÀ:ĚŸ˜·À<K¯)M×#@Ñ·gµÇ@AËÚ^…Ç?Ë´ge¿Í`?¶­¾,0
?æqËtÝø@ížÏ
™Ç¿çæüÞãOƿ⸝Ö?<V¿áF%žu "¿æ°Ì@Šß—¿ïü•aütZ¿ï¾áÝU03AGNbcuB3 2314+377?ïüCšú7?B:€Õs.?=ã(.GoÍ?B:€Õs3?ïù	¢†$ ?tYA©Ü
d?KÙuçoƒ?tYA©Ü
g?ïR@'Üv?en^îX	?•·ÿ/¤qk?en^îX	?ïܝ±ô.i?`Å€°·Ì?q±'èËÈ?`Å€°·Í4FGL J2317.4-4533¿îD´°-®#ÀOâI@¼À:/e‰Ç"À<Vè³³ @½EªI6?ü¯§r 0?º2€…Ì];?ÆǍȪÿ@'3@˜™is?ïþ.~Ãq¿à2÷~|1Õ¿ØTü܊%¿ÝTVc¹ã¼¿ã~¬ãù9<¿é^­'*AGNbll3FGL J2317.3-4534SUMSS J231731-453400?ïü6›¹ù?<è¢Üß'ê?>K"7È2s?<è¢Üß(?ïû›Zp•£?W²Ë2™ú?A'–=©v?W²Ë2™ù?ï*šKe,?–¯Ù Uú?žz¬¶"Zm?–¯Ù Uú?ïäõuóQÑ?Zo½¢|@?k
Š®/X?Zo½¢|B4FGL J2318.2+1915?ï9z$'›þÀC4t}€^_À9²Áo¡x‹À<Íê>y@ËO¤@I´˜c9?¶Ì—Þ-G?|¿ûûZ÷?Å'T,þ@,½£9+¿à\VbbJοæ–{(,¿é0¸.°¿àÆးø¿îE·Ï冿ïü;ºÁ1ŽAGNbcu3FGL J2318.6+1912TXS 2315+189?ïþËgP?&†
4ð¾ê?#I‡ê÷"R?&†
4ð¾Û?ïþLж!?FÿÅhz?+?¢ôÖ¥?FÿÅhƒ?ïݩڂ^P?r©¡Bàk?q+¾Ð×Ú?r©¡Bàp?ïþ¬ìz'™?ºéZ$?%18Væj?ºéZ#ô4FGL J2319.1-4207¿îǪܿ"ÀP|+IºÀ:uú=H_ëÀ<•æÉÎ@,ùÏdVÂ@.Øà×EÍ?¹oÛÛ£
¿ŠŽÈvÉ?Ñ«Dœ'x?ý6"y þ'?è÷Z_G
[¿ãmü\ÝP©¿à'Æ-Vпà…à19¿âW°ö­pç¿Ûâ H£ÞAGNbll3FGL J2319.2-4207PKS 2316-423?ïñ€'Ð]?Vòi?\ÿÔÜ_Eµ?Vòi?ï÷¸f1?eB<êÖ?Qõî3 ‡?eB<êÔ?ïæ__]"V?qµÆ´ßÄA?i  ¢Ý«?qµÆ´ßÄ@?ïʐULd?fqC[?z·ÕYÍ÷£?fqC\4FGL J2319.6-0456?Ú4ss6ðÀMkøüÖÔÀ:ü8ç¨fÀ<‰á<ÆYì@ '¦un?ú ˜ u?лR;Œ/?΅xdë'
?ÿ•S¹»@þ€G7w¿ï嵜.ŸP?ëýQÏÖl‰?•	i¤ù
¿Ð:n%wˆÎ¿áj3°0´Ô¿áI€|'!ÖAGNbcuNVSS J231929-045640?ïô ³zY
?UÒ4U-Œ-?V¾™MæA?UÒ4U-Œ5?ïü7Q2h?R.`ø·›?>Evo$±{?R.`ø·¢?ïÁF!7é?{˜83?º0?\ïd~ê?{˜83?º8?ïÕ¤%u?d÷dÔ?uxx-íE£?d÷dÊ4FGL J2319.7+1609?سàæóÐÀDªiƒQX¸À;/=÷²S¥À<¡ßòC~Û@ ¯´õj¥»?ùgk´"«?Òãk¿ì""?Ԕ–e¿ã@Á}ä1@düsÙk—¿ïþ›vóQ?ïòh!ýU׿垴‹g\¿¯>'iÈ¿á×U¼Ê÷
¿ïó¬ÐDÑAGNbllRX J2319.6+1611?ïù'¤MŸn?Eå3²=³ë?KanɂB?Eå3²=³Ó?ïê1m†h?'0·ƒÍ?eΒry—ó?'0·ƒÍ?ï±K@¼×6?€$‰÷*?ƒ­/ÐÊ2¶?€$‰÷+?ïvX÷˜?'¸ØÌœ?'4ü¬û?'¸ØÌ›4FGL J2320.8-0823?æë7'^‡"ÀNőÙýÀ:Ÿ>ÔI™À<Q˜hA1ù@j×9bL@2Á¾{Ñ2?Û÷Ü°ožô?Ú+ഐ@@¹áåéÔ@	P§d?ïûU@¤4þ¿ä©ÅÌ'‹_¿é€¾×@Ä¿ë‡Làƒbö¿ïõN`¶#=¿ïÿ%D]'#AGNfsrqPKS 2318-087?ïüëæ™òx?Jt<‡5œ¶?8 Ë0l=l?Jt<‡5œ±?ï╍'¬?€Ž·?mjrðØSk?€Ž·?ïhihÑ:?'8]o?ÒòÒåØæ?'8]o?ïƒsõ鑕?~U´81ÉÕ?#…›š'?~U´81ÉÓ4FGL J2321.0-6308?»i—¶=£ÀIŠiƒQX¸À;[ìëPFÀ<îUsÏÛu@ ;òÈ	­?ýDÌh"ÿ	?ÉX°›>?À¤ÿ§j"?ó홖>›F@nr
—~?è¿Wߣ¿éì¶wò?³
|%js¿áMÚ~f7l¿â>™˜ÂÚ¿âw®aÐ*AGNbll2MASS J23203986-6309181?ïùø"Ú'G?C{<÷z;
?H¬•¶àP?C{<÷z;?ïüö—EŒw?Q_ÿ0ö#£?8KEӜHO?Q_ÿ0ö# ?ïðß&â"?by=G¿¨?_øA²:×B?by=G¿­?ï܄A–Cz?]¹U 
(?q½ß4ÞC/?]¹U 
24FGL J2321.4+5111¿ÞêćÓ*À"hæŽ>ò"À:7{~% À<H¯¤Ùš@þI'¼1Ÿ@SüC²Ý7?¹2·ÖEœ?ha[¿¸J?±ww°»Ÿ(@dš´KÍ?âmy_èGý¿®e!0Á¿éõP¯Dü‰¿ÕXÅÉ£M¿Ñ¿

Áû¿í)\_§ZwAGNbcu3FGL J2321.3+5113NVSS J232127+511117?ïñ	ǔ?aŠ¹Nô?]ìp××ÖF?aŠ¹Nò?ïþõaþ8%?;È6qFt? ©à}­²?;È6qF•?ïÐ}>æÆ?{£ǔ¥?wÁ`ý ?{£ǔ¨?ï÷!µ¯
Ë?AH³±ƒ¸q?Q¼"¡äk"?AH³±ƒ¸]4FGL J2321.5-1619?æ?¶RðÿÀP¢øa¦
EÀ:2íÈÅ×À<PšíV°@ R""Fô[?û\ãJ½"t?¿']è¾oè?¸½ßÉÿ'ó?ü`q$/Š1@Òú›½
b?ïÆ•Q5}¿æŸCâ­ß¢¿ÙoD]¿ÇM»à~í¿ç€N9Hö꿧Û7TAGNbll3FGL J2321.6-1619NVSS J232137-161935?ïÿZ'Z#n?
Èlš+ü?¯´»'8h?
Èlš+Í?ïýá	ïr‹?M²1…V?0÷°"kŸ©?M²1…F?ïô.<³ã˜?aA¶!7$?W£†˜8ÍÓ?aA¶!7?ïû's?5à{íÃ_?C÷݉º3v?5à{íÃS4FGL J2321.7-6438¿î€~ÆÃ*ÀHì° Ä›¦À9µKÀ<p¨O?t@Šû"@ÈqGÐ?­;Ì´Îÿ,?G•๗%?'Õb垼@»¨pL\¿àp¦€Ýµþ¿ÞŒ'àl絿â>=Áç¿á»i˜JA¿å(ǟfb¿» ×»é$ÇAGNbll3FGL J2321.2-6439PMN J2321-6438?ïÿ'(¹C?9êÝ^?›è×Ҙ?9êÝ^Ç?ïþZþ×ÛR?F'‰ÙŸï?*P'Jޏ?F'‰ÙŸà?ïôI¥Py?]|7Tù?Wlµá_
`?]|7Tù?ïÿú¹z>Ä-²HƒçŒ>Çåð͚>Ä-²Hƒá4FGL J2321.9+3204?ÙÜ€á
À;ö<1ßvÀ87[‹ABÀ;‡³äžzª@Øם
gb@Hƒ&Ž? 'FJƒ?¿ò.±fS@ý"$½@Y0Eíõç¿£G>ÞF·¿Ýû†ß؝¿ãJ|àü.º¿ã¬fZ§ìC¿é袠ÿ>¿ëB&¶M.‡AGNfsrq3FGL J2321.9+3204B2 2319+31?ï¨)¼Ìû…?"ñe;?…õÌÁÙ?"ñe;?ïò/E¯ÈC?rØpîÔÇz?[¡t oyy?rØpîÔÇ|?îûaä`?•›3ó«à? Nî¹áº
?•›3ó«ã?ï÷,Ԉ\?DY,ýsþ
?QŦVïI©?DY,ýsþ4FGL J2321.9+2734?å5—À?;Y5ü;OÀ9"¸ÜU
À<4›ök+È@w>ÿ¥@¦pâÁ*Ø?³¤ëÝ3L^?¶Y"€a'@³â…›µÔ@ܰљ4?ïåѶ@™M¿Þ¡NÄ´$Š¿äœ<I	^¿ÜmÍ"ˆ8¿è˜¢ô¿åt¦FPFAGNfsrq3FGL J2321.9+27324C +27.50?ïËÙص?|Æ'ÆÂ?z÷%th?|Æ'ÆÂ?ôï'x?¥¯;	¼u?šÂÄ¡Ð?¥¯;	¼u?ï>ÅÎqq?"yFK{?˜'F1ÜqÕ?"yFKzÿ?íõ»:‡žH?•ÈÈV®'V?°R&+Ã
²?•ÈÈV®'U4FGL J2322.1+4440?ŒRËÀ.·¤ƒ§ À:©È"h¯íÀ<\§D}"@Çs){r@'ä´J?Ë}õ#XÐ?ÉÓQáŸÜ@]týØÞS@þ#ØÍ6)?ín«äõ¸~¿ÙpfÅ[ê7¿æåà/Ò¿ßnwa¶Sd¿ìðZÛî¨À¿ïõ_¯"AGNfsrq3FGL J2321.6+4438B3 2319+444?îœÒA®n?¤Ù"…?¦2Ûå?¤Ù"…?ï6›«j?³?ªµÊ&;—æ?™,Š'¸	Ô?ªµÊ&;—æ?ìÅÝéyž?¦¾^ü²Ö>?¹×á´3?¦¾^ü²Ö??íñÿ	¥ ?—¼°R?³xp²Ó?—¼°R4FGL J2322.6-0735¿ëThÌ0ôÀN¤gbèÑÀ:|©B"	À<Vhiuå_@+ëÞ
ò@bå€!ùO?Ä­Îq?²½)썇h?ìrAÁ@|@|e´å¥a?ïÿT>Eµí¿Ö7@¿åº#ý¶#¾¿äc4^ÁV¿æ6_½Õ¹¿ïÿÀ_V&ÓAGNbcuPMN J2322-0736?ïÿAÚoQ‡?t;7ã?IJÏC‹?t;8¨?ïþÇ4ts?<ÅÎðs?#Œ¸¸ÇB?<ÅÎðs>?ïÝ´<ì—?pyÊ2¦e?q%áõ‰³¾?pyÊ2¦^?ïþ±i«3?Äöp— ?$éeLÏä¯?Äöp–é4FGL J2322.7+3436¿çoAL‹GÀ8Ê!§´ÝÀ:ñ
™¶öÀ<T_°i¿·@ 1͒ð] @'5>¦?²Ûù ÜÚ¿¨›ˆ²¼U?öôÖ¡aä÷@BY@ãö¿èŸÁ¦Óê¿ÝçK~-­b¿å§Éþ;YÈ¿Ýu=äçöŸ¿ØºËã˜Á-¿ÔÔúc
AGNbll3FGL J2322.5+3436TXS 2320+343?ïø"ÖU¹?K{¸+ï1Æ?O¿t¦©‹?K{¸+ï1Û?ïýÍΐ2˜?I]`cý?1'‹~k@S?I]`cç?ïë¦ØD"^?r1mû62?dY'»k¢l?r1mû6??ïâÐÇxLº?Yß)‹±ëÔ?m/8‡³FO?Yß)‹±ë×4FGL J2322.8-4916¿™Ë˜FUÀO´á¼©À9ʾšÚâ9À<
¦{)l
@‹]"•{}?ùÉ¥¶Žj?¹­®#"Y¿?Æj Û'G@ܸŮËZ@ã¸>Jh"¿ïý2%9þ?ïÿ"D¾Â¿Ô¹`¿'F¿Ñbf¼ønf¿åǞ?È¿×pŸ$rüAGNbll3FGL J2322.9-4917SUMSS J232254-491629?ïøåΈn?JiBWÌt?LhÅÞGöà?JiBW̔?ïë2]¥…?›'{ªÇ("?dîÍ¢Z{p?›'{ªÇ("?îç©ð…ø?–Å­Äb?¡Žµ`÷ Š?–Å­Äb?ïÊ£?l½?o'à£·c?z®r`I¡J?o'à£·f4FGL J2323.5-0317¿æjFDj(?ÀMO½­uÀ7勾åƒ}À;~^ÛWª@¿ÈVÆ`L@HAíá?šo7àü®?¸''	"83@¡e}'%@Éï"µ¿ÑTù²W¿Þ¸ô¾-w²¿ä¡:B-ƒ¿äxfÿš6¿éÏ¡þÂé¿çÞ7u¦AGNfsrq3FGL J2323.5-0315PKS 2320-035?ïïêk»Ä"?UÑûŠþ¤g?`"D;}_?UÑûŠþ¤d?ïìYé)ü?^SG¾?c¦bÖ5?^SG½?ïŽõ®eÙ?tÕî2?ŒB"f½	×?tÕî2?ïú
ËÐU?:Q,©ċ?E‹Ôо­‡?:Q,©ÄÕ4FGL J2323.6-0617?¸ÚÚȲÁüÀNBàP7PÀ9õ¸Ú§€ãÀ<àŽµ:@‡|"P.—@é=¿Íá?»ðN²º¢?ÇR¿€#@	ÞRù¢í@׵̀?íri^¾Q_¿ÚˆüvÄ¿ä˜Pž¨ø¿èˆ4ýbÁÁ¿ét÷Ãñ[ø¿ïy
]QïAGNfsrqTXS 2321-065?ﺍ"wx??ZŠ
†£?\šâ!ùÏ??ZŠ
†¢?ïýQŸ"Pb?NñÐu!EÐ?5sÝ|ô|?NñÐu!Eï?ín\;Fy|?¤OèDõv'?´%Ì4?¤OèDõv(?ïþæ=ïp'?'u,\ ?!œ!÷3?'u,\4FGL J2323.8+4210?瀁ÕoÒÀ1ÍýÞ½À8«€U¾À;"wï$æi@L{)#Ù?ütwéR?¥ÌÁ¶2?±v¡G
Ë@.xžwNì@
Nv/²¿Ù#¸ÁÒó­¿Ò¢Ÿý‹Üm¿àJg,_œ¿Ö(ÑE'пÜzptb¿âÓ¿°.±AGNbll3FGL J2323.9+42111ES 2321+419?ïý˜Î€Ï?'•kçP6Y?39‹ù‡w?'•kçP6h?ïñ	³pZ?{›+î}Áh?]ì™ïKB?{›+î}Áo?ï߂tnO7?u~傔ì?p>ÅÈØdê?u~傔ì
?ï΅Øiü?b>"nñy?x½Ë|~?b>"nñ}4FGL J2324.7-4041¿¸:CqdJgÀPå6&,ºÀ9+þ¤¶-NÀ;¼çºŽÜ§@Øc1R³V?ùùÆ_ËA²?³1`n™€?µ©¸J´¯@å:a$Þ@H€ú?ÁʹÍÇè¿Óf$a´%¿Ý±äíU¿ÓryšÑW¿ÙÊûçA˜¿ÖìsԐAGNbll3FGL J2324.7-40401ES 2322-409?ïþ@8‰1?$;zX"Ý?+üwf,æò?$;zX"æ?ïýÀ®ÇRè?I|µ‰ž{?1ú‰Åh¾Û?I|µ‰ž{?ïæ7ôÆÕ?oêqÄùÍ?ipÈ9+Û?oêqÄùÎ?ïü`	À?1‰–Lü??ÏÌÿ±òÇ?1‰–Lò4FGL J2324.7+0801?ßµáŸjÀH†`˜À9'‹©ìÍôÀ<$_iòâá@[(+îz@"­ÿ'+¿?´¾¿iŒá?§k,Á "–?ñY×\rǞ@	Yh&/¿äƍm;¿Þ4ÓpsÛ¿äßd¥Ï2¿Ýx`«¿æ¤"…|+¿æòø°€eìAGNbll3FGL J2324.7+0801PMN J2324+0801?ïü€ð¼îŒ?3
B9V!?;øz‹¡Ç?3
B9V?ïýú,¢ù^?HΦzepþ?0.šè5x?HΦzeq?ïóÀ2UB>?_YÌ)?Z?X›U{ƒy?_YÌ)?F?ïï¾?÷'?QRìÔzsÂ?`AÀâoA?QRìÔzsÀ4FGL J2325.2-2010¿ê&z²ŒÄÀQF¿]xÀ:ú"=_ À<¬˜ÜÛ7Ê@ Q$"‰åG@Ûþ +ïr?¾ôöŒŽÄ)¿´C?šÊœ?ó$5æ€Ó@"†ÔE,?î:ߎñ¿åM¤c!7ˆ¿çti>2пÕMW—Õt¿Ö(`¼ƒS‡¿áæ7¢-¼ÒAGNbcuNVSS J232520-201213?ïþ,Í6Wé?"ŒL''éÚ?-3,šŠ0?"ŒL''éç?ïþ"Tÿ"j?Kig;õ— ?-Ú°¹e?Kig;õ—²?ïùÖfƍ?Vوôè¸Ø?H§ºdåː?Vوôè¸Ú?ïøº'™ñ??œ${âýÓ?M·é˜?9??œ${âýÎ4FGL J2325.2+3957?Ðj'7Á)²À3ûªy»­ÁÀ9	Ô¿	•«À;ßʯ¼Î@^(ÿI!?ÿãiÇCöÐ?¨É&O"?½–­@Zöƒ{á@GS&m§ù?ï)KRä©¿½§A"	?D¿âáÝ Y§;¿à—[µ2|¿ä\ËG'	¿ì
³!9AGNbll3FGL J2325.2+3957B3 2322+396?ï÷¤O¾"w?V#Óߧ£¹?P·`ƒ»é?V#Óߧ£Â?ïæý_× ?{ö2‰	ß2?i ï(^¾?{ö2‰	ß1?ïYZS!Χ?50_ùD?"Ôµ›Æ++?50_ùE?ï…~W ò3?t|m{ìÿ?Ž jÃrï?t|m{í4FGL J2325.4-4800¿ïVpš6h¬ÀOž¡ß¹8›À9)ÎPZ‹À< }ðƧ@"E³"@ƒV–åŠ3?­RŒâŽS?£T<ò½?õc£Âˆ@2ÃÈí¿Üƒ€Þ6׃¿ánðx£Ì¿âÿ¾øMڿߜè"éŽú¿âár@<I¿ãY¯åC;AGNbll3FGL J2325.4-4758PKS 2322-482?ïþ\øäœ?$…æéo{d?*0vñ¶5??$…æéo{h?ïý½Æv=¬?I"ÒE{Åã?2ÌN›¹?I"ÒE{Åñ?ïôj'Ô?cTªôts?Wã+±Ð[N?cTªôtp?ïüjÇ8˜x?1#+ã¯Ñ?<©Æ;<?‰?1#+ã¯ë4FGL J2325.4-3559¿ÃXOñwÀQmƒùdoÀ8ö¬Lú"–À<¯Ù`Y@›©ä'@á%Ie¥?¨dË܌ÞJ?Ç:`Nq@jG¾²í@\¥°ÔÏ¿ÓÝåC;>¿ÛêÆ}'s¿ä€!Î\¿ç1¦k94¿íRCÏb©C¿ïÿ¾ÿ"°AGNfsrq3FGL J2325.3-3557CTS 0490?ï}¾ÄT?¢¤_`LŽØ?Ÿ°\È'u‰?¢¤_`LŽØ?ïÁƱ²Ý?¤(t'È?§&'qH?¤(t'È?éî^FõŒ?²	š÷~6ì?ÈF†ä)Ïþ?²	š÷~6í?ô#zÇ?zdн]Ë?‹Ò'÷!Mè?zdн]È4FGL J2325.6+1644?åydw˜'ÀD¹Bá& À:º$?ziSÀ<ƒ»ðÜvŽ@ +Wdë¼ý?þÖ>J¾j3?Ãrµ)B©?«kÿœF·?æRm —d¶@vӉ)‰ç?ïý¢È6¿Éo8&&Z¿àqkè†f·¿âžüå™Lm¿ÁÍ=
!—¿ïþb †ˆEAGNbll3FGL J2325.6+1650NVSS J232538+164641?ïÿ?+un¿?!×ô×E[?'R(?!×ô×E'?ïýﳁí?OH¶ž,¿^?0'gCð™>?OH¶ž,¿d?ïæ–eˆ!A?q3(&œè?iišwÞ½Ð?q3(&œè?ïùN*"E#?<G/ﭐ?JÇU²ër­?<G/ï­¹4FGL J2325.7+1821¿Ëã'ƒˆÀCþwÿuÀ:8(y›ÍQÀ<NÌܽ@Т=­	¹@ÃåZbL%?¶(™Ò#¤¿­w?ö:.?õeU	FП@	Cü ÍU?ïçǟ'UR¿äéŸìD¿è´áMK¿ã›ÔÝ<†™¿ëQ©A­?ڔ‰¤Ùé–AGNbcuMG1 J232550+1822?ïúÓ¶ë1ë??ùSFš1×?D±$S8Ql??ùSFš1Ø?ïüâ»ôQ$?TçR|à?8ê ]vâ‹?TçR|à?ïÚÚNä"c?vgq$fÖË?r'؍½Îù?vgq$fÖÊ?ïñWûç/W?I¼¯OP?]P1¡S?I¼¯OP4FGL J2326.2+0113¿ÙÄ"¥/˜ÀK'ËûµtÀ:ÄfõŸ<À<"Ýao†¡@ºø"æßÈ@ü¸oG¶?¿˜p_õš2¿wåh£M9©?¹¾|§ñK1@bÁ5"âP?ïÌ;ýÝ¿×ø¾BEtÔ¿ÝÇ-ügš¿ëö>¶4ž?s"Âïö"ê¿ÑÓwá¸íAGNbcuSDSS J232625.63+011208.6?ïþžû
`O?${&Í¢?&OYû
D?${&Í¢L?ïÿ1gÛÉ@?8o>ÃE'?Ó†×ï5?8o>ÃEK?ïäÔm¶›?'b {œš?~-•É$²,?'b {œœ?ïÿáÅ\r4>å
°ËèKG>î:£ËÕ×>å
°ËèPÆ4FGL J2326.9-0201?Öã,Oñ‰ÀLàyåŸ+ªÀ:e^ɹòÕÀ<""ÍŸ@Þ~Ðëj@/FÄàoA?¾ŠÀÏ¿¤«@¹ûÜ?äöÞ¸1µ?þ$qÔ®˜"?ïInÞÛ¿å^m=ðüW¿çº•"<¿éøû^°¿Î)F Mgè¿äC¯'9+AGNrdgPKS 2324-02?ïåaè©ñÁ?g"Í"sîÇ?jžV>.?g"Í"sîÌ?ïÙØ9>"®?‡Ø~Ö³ðs?sã`î§ð?‡Ø~Ö³ðs?ï['šåˆ?Œy¶™Eà?"¬£_.ý?Œy¶™Eà?ïč9 ¿°?lËf΃*?}¹co '«?lËf΃'4FGL J2327.3+4717¿±*dc{qÀ*h–š
Ø¡À:·V¥ÿªÀ<~¦ã@N´C%?ý÷})÷JO?͈ܲóݳ?͏¸š:Ô<?ýýI‡2ŽÉ@X;¯X¦?ïãĕƦB¿è¨Ö]š9ý¿Û"oH7Œ¿ß}…fÜ­ë¿ä± VL<ï¿ïýB äfœAGNbcuNVSS J232723+471601?ïi?`=dž?ayïqø—e?`=dž?ïö)Xæ2ä?fõAnbCO?S­N3š8o?fõAnbCG?ï?Y`'@€?'a-óæ|)?˜Óûð)?'a-óæ|)?ï1±,Ôû'?~œø-oƒ?™ÉÚe`´?~œø-oƒ4FGL J2327.4+0444?è"
âÿšÀJ"Ðå`BÀ:Øÿ€¾À<f"Xð\@ëâÈÇß@q…Æ}þ?ÃX"ÖĝS¿™."hƒ?ÍêñûÛX+@ùB·Š›?Æ3h7Kñ›¿å.·£oÜ1¿åÀBŠ3ö¿ãdŠž›¿ì4üa'¿ÈK4Ä,ëAGNbcuNVSS J232733+044740?ïõn¥¤Šû?Q\¥ý¤?U"´¶êW?Q\¥ý£?ïüê«^ãe?P£VŠiœð?8ª¥äâG?P£VŠiœð?ïÖxçéDô?yÏïW1+?tÌ]…Ð?yÏïW1+?ïúÏ«œ}/?5'cO?DÁQŽAè?5'cM4FGL J2327.5-3259¿ëßƛ¡ÖBÀQ½Œ¨À:·pÔ~qöÀ<­æcvÇÝ@ø4O'åJ@3fÿéYË?Ë:Ïç/O?Ȃ;òŸo?ú'(bõ˜ž@¶Œ½¾?ï.Ô>[/|¿ÝzX@ˆÜ2¿çU~¢u¿ée2`=W¿ð?ïÿãåîAGNbcuNVSS J232747-330130?ïþ²žÁNƒ?'Qx+çõ*?$ÖëÉì?'Qx+çõ?ïø—äö†Ã?fj@ï?M l%äô,?fj@ô?ïE5cC—?Š‹þJ¤öS?—Y\s—?Š‹þJ¤öL?ïïFÅH;?Sÿù)œ´&?`¹:í·Ãõ?Sÿù)œ´4FGL J2327.5+0939¿ïû{jXWvÀGü£a™xÀ8¾®×ï?¾À;§:-ù7@w"ìá•@tõÅêZ|?©4'yì€?ÀV:ߤë²@'bØ<l˜@µÌCŽ¿Ê
2îà¿äõÿ 1#¿éŸ¿™£¿è™cé´d ¿í‹Î2JU¿ðAGNfsrq3FGL J2327.7+0941PKS 2325+093?ïþ"¼þuÅ?'"ÏïGÊw?&Ä0£¼¼?'"ÏïGÊu?ïú',eè?d‡-šò–)?E»ëNhi!?d‡-šò–$?ïtôÇ[‡9?;a*ÏÛû?'agÉ?;a*ÏÛý?ïü®¡ç?5J¨Htâ'??bŠðÇJ"?5J¨HtâÆ4FGL J2328.3-4036¿è?̊¨ÀQ
-à
qÀ8•t/|ÅMÀ;¤BW"dÌ@—);¸'Ù@©Cäõ?£–œÂ¡ƒQ?²½g4@H/yjO)@ǶãV|?Èd¤Yæü#¿ã²úÉ_Z¿å5¥Õ?¿ä%'(]í¿êÅ
á?¦¿áĆ!—ªVAGNfsrq3FGL J2328.4-4034PKS 2325-408?ïøê×I:P?C²†º©?LT¢ÛÃú?C²†º©?ïü¦mg4?Vy0 @ó,?:̔Æ_'a?Vy0 @ó3?¼¤y?Œ>U:?¸PÖá¡?Œ>U:?ïýÇu?&
+)P@µ?1ç3ÄW–?&
+)P@¢4FGL J2329.0+0832¿î˜ëmãÂÀHúÁҝÇÀ:X‰ÀßÀ;ú"õëª@	8BÆ¢@¡Ý»1™Ö?Ç/Úx±íx?"%îbYø€?ÆN³×³Z¶@ãçiܹ¿ã6|=鵿êMf»ü¿çµL»šu¿àJæ
²û¿åéázÙºò¿ðAGNfsrqPMN J2329+0834?ïþ.¡k¢œ?(ΤtxðÊ?-éEÖ1@?(Τtxð`?ïýÉCî˓?Ué@î?1µà‰£\ñ?Ué@î?ïÙ0ÑEr?vΩ'Ñœ?sg—t]F°?vΩ'Ñ"?ïù—x`?<Båšf?I¢ÓÒ~A?<Båšw4FGL J2329.2+3755?ÒÐM™›6À6(ö¾7ޔÀ9œÏýÚÀ<ÂVQEm@ LêÇϸ?þ"]"<?±K£—tP_?Œ´íTy u?܉ݤ`r@"UZ$Ž«?ïÉÁ_[ZD¿â	€,A¿ã&pA±{8¿Ôúv=Éå¿Þ›‹Œ;¿Øp¹[UçAGNbll3FGL J2329.2+3754NVSS J232914+375414?ïüžÓôzÇ?3‰,	¥V?;	`\)È%?3‰,	¥P?ïþ:ÀK¾C?J‡·Üý?,SûDÎn?J‡·Üõ?ïðAãA¬?eù©"mº^?_}ð9|¦C?eù©"mºT?ïçxBØ?TTîƒóŸf?h‡ÿ½ô)!?TTîƒóŸr4FGL J2329.3-4955?àÝð- ªÚÀO'L Â'ÇÀ6×TûÚ×RÀ;A.jv–_@¾5°;@iÂÝ`?‡­ºÚôƒ?»֑ò†@,úuFÓùè@"ùÃǕ€¿›oðAµÆ»¿àe•P^½%¿äâb`Ght¿åšÅ都¿é°
Ÿ@L¡¿ïHG,{ÄAGNFSRQ3FGL J2329.3-4955PKS 2326-502?ïá«M[´€?d$SJFvÅ?nT²¤KŠ?d$SJFv¼?ï½­jÁÀ?–ÙÐmÿ?€"¥O :?–ÙÐmþ?ïáÒnþþ?•uäC¼P¢?œŲ  1?•uäC¼P¢?ïÚã	·£?uü
Vš¹ê?röŽ{$.-?uü
Vš¹ì4FGL J2329.3-4733¿ëº'µ3ÀPÂÀð À:FM½"4ÞÀ<P!ÀD(N@íb ®ì@ä1æ,c?¿ËÜ!~ã?¥añÆ\Æ?âùåŸ+©Ò@:-1;ŒH?î>rο济¢o¬
¿æ—"[tšÝ¿âh>Õ¿ïÿªÅÝð¿ïü»!©ôAGNfsrq3FGL J2329.9-4734PKS 2326-477?ïþsŬÒh?%|UV?(Ã¥2َé?%|U[?ïþ‹´«Œ?@5:ï/?'D¿G7ë?@5:ï?ïà
úÃù¶?sË×Т?oõ<Ic?sË×Ъ?ïû	ðãMp?5b1ÝÖù?CØ<rÊ?–?5b1ÝÖê4FGL J2329.7+6101?ïÖ.²s©.¿Ò׳ϝÀ9"å'–pÀ;Â`{jÚi@ ÷u½qe?ÿ9  ?½X¡VÒI¹?±½wg?ó·
1A@9úÄ+éh¿äÛQàG}î¿ÜÑT
H¿ä=Ýܽ¿ÔÐß´0¿äÒ÷S‰¿Þ=Á¬ˆ4AGNbcu3FGL J2329.8+6102NVSS J232938+610113?ïýÕø¶Jó?0\»èñØ?1P:M¨ek?0\»èñõ?ïá̳ôg*?"fÙÀ?n3L˜Ö+?"fÙÀ?ïÔXî÷ƒ?~µt`6wU?uӈ"9>î?~µt`6wU?ï¸8½Lå?sÝËÒ´ñ?ñЬƻ?sÝËÒ´ï4FGL J2329.7-2118¿ÔûˆÿNœÀQ âe+ÔÀ:ÚJcÑaÀ;홭»Ž@Ù"˜€•@¾0O‹Y?ÂÏ
¿¡–¿‹ã­'Ú©H?Èô{§ìÁ@ï¶wö±£?ï²ÌÛæED¿ë棣×e¿Õ§¢Æ¾ì¿éÍÛU%ÌB¿âQ7@¿ïù˜¨)AGNrdgPKS 2327-215?ïÀ}|ô›?zÝ–ì¾?·ÁA…²›?zÝ–ì¾?ïñŒ§¨Y?s2€ÔÌÓ?]Âæ°¯O5?s2€ÔÌÒ?î«ó,õ¯
?—á{쐵Í?¥@Í0¥[?—á{쐵Ï?ïŐü	±ª?mê¯$W¯«?}7û'+S?mê¯$W¯¬4FGL J2330.2+7759?çu%'Ðù@/œŸ"…]¢À: ÝU±}À<]pŒZö@ý÷ºa:X@⿐¤(?½¦´4P?¾wðýX°Æ@@Äe?@
~åkT6ä¿ãïa·ªü˜¿æE¿ý±q¿ä•[Fw´¿ã‹B¸â¿è‰ýÅ=6¿ïý«Ç™‡%AGNbcuWN B2329.2+7743?ïëK[°Ü?džyÊ¢A?d´¤Oo$ÿ?džyÊ¢9?ïù7¯˜ã?cÖ¥ÿºë?K!AÁœvÞ?cÖ¥ÿºé?ïË&>&nî?w~@
÷Ül?zlàìȉ?w~@
÷Üj?ï뻬fJD?Pïi5+Ø?dDS™µ»a?Pïi5+ß4FGL J2330.3-2332¿ÏQ¥õàòxÀQÖ"t¼jÀ;t‡'YYÀ<¦ÞãOÆ@gÄW]_@p Ç`?Ò»ûS?¾P[!¹¹?îրÀ.Ù²@d.'Ü¿ïõúÐ7»?î;¼(ßó¿ç"€$þg¿Û#ð_£ÿy¿âý²}–-Ô¿ïÿ?…¦óAGNbcu2MASS J23301617-2336413?ïûëú9²?E䞊Š›?@SÜ6ž?E䞊Š–?ïëlٔa'?~ÕÜ´¥ý?d"&kžØæ?~ÕÜ´¥ý?ïÔxl¼â‰?tÎJuÍÛ)?uÃÉ¡Ž»Ö?tÎJuÍÛ2?ïÈ­-91?om&1?{©ic8gÌ?om&1	4FGL J2330.3-2948?çbõ´Ç1àÀQÿÐR"JËÀ;Ñx-8GÀ<Áû
Qø@`ŒŠ¸Ö@sgÁLf?»Ío4[\¿·–Õ™úèi?ú#=ó?è›$T"Lç?ïr-^ÝÛé¿â0¶¶àÒ=¿ä/?› '¿Ú©A­Iz¿Ûh¯a,Ü¿å&ÓßÅpAGNbllLEDA 3230048?ïÞ¥cokÞ?¬;4±·Ð'?p­NHJî?¬;4±·Ð?íßܜ© ˆ?À½ŸL¿n©?±²ûÆ?À½ŸL¿n©?ïƳ¦šà?€Ðo×c{?|¦p,²Ó?€Ðo×cx?ëÉÜÒÎÙ?«rðDGÕ?À؏"´Äœ?«rðDGÖ4FGL J2330.5+1102?ÖÝi©ZÀG‰c4'¾ŒÀ9úŸg8ô=À<¯#nš@ZV'©è@õNÂR ?Ç<5»MÉb?Ñ{Pw@ //˜t@
V¡¢Q¤¿Ô	 ØÅ¿çæáËâl¿ç\Á¡ö_¿îWšPx¾X¿ïÿÝÀåãÊ¿ïÿÿ)@k*AGNfsrq3FGL J2330.5+11044C +10.73?ïýúÑc!?3j_XRká?0)tæ÷y¤?3j_XRkñ?ïòË0îns?p¾,'Ø·?Ziž##
?p¾,'ص?îAŸAx?›'ÂVøj?«æKît?›'ÂVøjœ?ï­¸è1-?rÝ
ι
T?"'Åó´¿²?rÝ
ι
V4FGL J2330.6-3726?·G¶£‰'ÀQ‡ ù	kºÀ:MµåçPÀ<=æë\@'"Æç@#¥™'¥?³çW'Žž¿±ÑÅÁ&¿?üûÅÃď@6càÐ÷?ïNË	~.¿ç	ÃÞ;µ
¿æu^¡ví¿åw¥[Zš¿ÙUÛ}¿ž¿çŠÄê€;ûAGNbll3FGL J2330.4-3726PKS 2327-376?ïîû((üþ?bÕ_Óñ?a×׎?bÕ_Óì?ïñ'Ào?y[|ÄJ;?]Èú!ì ?y[|ÄJ;?ï¦ppR.?…÷"E`ªÕ?†cãëti?…÷"E`ªÏ?ïÑ×}À½?f§ÌÎä/ü?wAù¡U?f§ÌÎä/ü4FGL J2331.0-2147?åf#µ÷òÓÀQ¾5'Ì÷À90b°Ï@À;ª"Xð\@BÏæ\ÀË@v´âË;Ó?°y5 W?À³³á™b'@c™,ŒP@¹@ÓÚ³¿Û9Î¿Öï=Û,áà¿çñZëÞàÌ¿åW¢žzÿÑ¿ìÛªëÑtÒ¿ïÿyB=KAGNfsrq3FGL J2330.8-2144PMN J2331-2148?ïòýwßjÔ?WbOݨ©R?ZA*Vï?WbOݨ©T?ïûhì$â°?]1dLõè?B\OluA7?]1dLõá?î I
`?›üG7KI‡?­ûo/¹ÿß?›üG7KI‹?ïù³ÜˆAo??R©÷³ä?I0ÞúBE??R©÷³64FGL J2331.1-1653?ÝØËGLIÀQ3y¦µÀ:êDrØ
À<G¥rë¯ç@¨+i:V=@
˅¤ð?ÔØ[
è'N?³
f
uú®?á"	¶@të¢%p¿ãT°',㎿ºcß½.8¿è7=^ZS^¿ìë»%_5¿ïþ®[È}³?ëUI°ÎjAGNbcuPKS 2328-172?ïÿÄ©\ÑÑ>ÿ_yAv
Ø>ý«Q—Bä>ÿ_yAv
K?ïðk#`©#?uÇTâ]l?_)¹>­ºþ?uÇTâ]n?ïsIjÝ?Ž*CyE-¢?'–Ò¤]I?Ž*CyE-¦?ïùÑ1­'¹?>ê¦à>©?H»9I¹X?>ê¦à>Ô4FGL J2331.3-1558¿ïº™^/ŒVÀQᛐëÀ:¶ÇǪNÀ<TtûTŸ•@¥¶Ê,@ÐE AY?Ð6̤?®ÆßԈÐ?ÝW¸"Æ©r@
³‰‹"ƒ¿ÊöZlˆ¿ëyJ]¿ßUûļ2¿ê†^¾Ò8G¿á(&à>™™¿ïöÕ´ÒÛAGNfsrq2FGL J2331.8-1607PKS 2329-16?ïÿ?Ê2h¶?#8;p,?¹²éQM?#8;nô?ïþbãº]ª?F{Í;<T©?)ÑÄZ%aW?F{Í;<Tž?ïǎÝKic?
ÚØ­ÄZ?|8'ZKN?
ÚØ­Äf?ïþp$‰A?¶;wœ¬¦?(ý¾—kÿâ?¶;wœ«Å4FGL J2331.5-0258?ëx®+I2NÀM™ìòù‡À;m/®CuÀ<'Ô{ø@ §6…º?ú¹Ð¦v ï?Ó¿²ÝãJ"?Ш $ã1?ü@j‰
Ö@kù«R(Â?ïò6H'iI¿èßvBQ‰5¿Ì/¥ßøù|¿Ù(ë܇ç¿Ðki$Ü®A¿ïÿÿ" 5•AGNbcuGALEXASC J233112.94-030129.9?ïÿ»,ìĖ>þò‰¼æG?4ÄÎÚQg>þò‰¼æ~?ïþUa†
B?Hû˜ð¦?*©çŸ[Ñj?Hû˜ðœ?ïÓ$H.?w›½@з)?vmø[èó®?w›½@з#?ïú<{û§?<Äáz€?GaÆâ?<ÄázÖ4FGL J2332.1-4118?ÕºîŽ\ÀQÎþÖ4UÀ:ÇÑ;ÇVkÀ<{èxú½¡@ûs'
@݇»¢?γ$Z'hÐ?؆~ŸBP@¬}Cø}U@"E¬/ô¿îß´tç?îa{zÊ¡y¿Ú@H%©ˆ¿éeDþ6Ò$¿ïôZ 4"[?ï­¹¬^˜<AGNfsrqPKS 2329-415?î XÈÛèì?«òW3eŽ?¥úsrAq8?«òW3eŽ?îxb™¹3¥?¹Y?}?¨yÖdlź?¹Y?}?êÆFYð¦ÿ?©\'—.?Äææ˜=d?©\'—.?ëä;ŒŠj?±'÷Ý9?¸?ÀoÍ×þ]?±'÷Ý9?¹4FGL J2333.4-0133¿Ïz~âP¿ÀM)¬îàóËÀ:¨Ó¶ËوÀ<	Äf̽³@¢PE½¤f@[›Äí{?Ð<}>šœ?ÊuqǬ?ú]­	¸æf@dõu|Y¿ïh;ibš?ée·ýä¿åž¸‡›jT¿ëŽäŸQi¿ã=ÓLKˆ¿ïÅ¡—ûAGNfsrqPKS B2330-017?ïÙÚz;}W?z¬É>}²?sÂâATw?z¬É>}®?ïðL4-VM?{Åq(¹?_g—¥Seù?{Åq(¹?íHÁ"ù`?§¼#{U"/?µ¹óØ4û?§¼#{U"1?ﯪfn®±?v[¨9"â?"fdTSº?v[¨9"â4FGL J2334.2+0736¿æÀ!¿âÀIGFýëRÊÀ::DŸlAÀ<3ßTŽÍŽ@}³Ö†´å@ŒÏ¡"c?»ñ~‡ðNÝ?°`u¶uY?í¹Å‰¬Ü@uu‹u•?ïÿyYˆ¿Ùjh~™Ž¿äƒÆÞ÷Ö¿ê${àK.Ò¿å'XýÈ[¿ïÿúŒ"¸'AGNfsrq3FGL J2334.1+0732TXS 2331+073?ïÿy'6¤?~ñBg÷?á¶2V˝?~ñBi?ïýî«GGÕ?J :ÇHšÁ?0Š¥ÅÁRÒ?J :ÇHšª?טּçÈg?*¤Òéð?"ÑÆ
æ:ü?*¤Òéî?ïþƒ÷ú:È?½ŽðŠŠ>?'À€\SA?½ŽðŠŠ 4FGL J2334.8+1432¿åáا¨§iÀF1(bõ˜žÀ9|G6v¾À;ïXÒÿìµ@XjGFˆ?þl»o?®Ï†C.0ž?¶'Ëïت@æ¥×Û@;FY€¤Ö¿ÀFdé8¾8¿Äa¦ù~†™¿áéàÙÊQ¿Ü÷jU¥#¿Þ¦YÛéuO¿î$…á*ý°AGNbll3FGL J2334.8+1432NVSS J233453+143214?ïþ†G)? '³•‹ƒ±?'žn[ç? '³•‹ƒæ?ïýÌ¢Ïym?JŠÙ•ç‡<?1šé"4'S?JŠÙ•ç‡?ïÀ‰Ë&Ô0?j"ôÌiœ?»l•èt?j"ôÌi–?ïÿ(2˜§?ÉùÌL?üY¬êÜý?ÉùÌM	4FGL J2334.9-2346¿Ù'j;M³´ÀRÚøßzNÀ:$Ú¯ä^ºÀ<aJ©q}ò@ÎRв_Ž@ܹ>z?»)9à '›?ŸÐb¿¤Œ?à"´/Gh@®òÇ2Y?ᅴ÷Aë]¿è%5y^¯¿æª>,‹y¿äùw_Ýá¿ìxá=G3¿ÏüƒHÊI:AGNagn3FGL J2335.6-2342PKS 2331-240?ïøà#?Hùñoù´'?O›"°te?Hùñoù´?ïüb$ÓT´?ZÒç†â4?<îÙeZi¡?ZÒç†â4?ïâ¥[.?ok\ïÿі?mZ¤bóÑõ?ok\ïÿÑq?ïô<E?FËò¬°M?V߇×tÅ ?FËò¬°-4FGL J2335.4-0128¿ìÎ셭vsÀME>>)0{À:\+ŒuĨÀ;öȋ­@]ú͑ë@	Þu?Ěº@ƒ'è?ÓÖX¼¯ž>@
tBâӟO@´r€s®?âUT€_὿ä‡"Ô@^•¿å°¤xí¿éëâ§)¥¿çç™!#¼¿ïõQ@9AGNfsrq3FGL J2335.1-0133PKS 2332-017?ïj°Èi?¡ú4¬$:'?Ò©æÿ³?¡ú4¬$:'?ïÑ£…õã!?£N]ÇӒ?w.=o¹?£N]Çӑ?êsÉ'ل?­¥Ð¢êº?Æ0Ûc°™î?­¥Ð¢ê»?ïwR…U&?y¿9p5?ˆ¢+^ª¶f?y¿9p44FGL J2336.5-7622?è5jóð*îÀCõ¦ZÀ:d"j]kìÀ<‡ó×ӑ@Ä%4ÂÕR@«ÈÛ¦"d?¼¸€uÂ`?"þcGÍõ?Ôà´`Dc\@¥¹z׿è7ŸS—Ø¿Ï"na‡"n¿â2/ýô¿å"~Z#¿ãÞó`4s$¿å"à\÷RAGNbll3FGL J2336.5-7620PMN J2336-7620?ïúåt!Ì}?BÄì'?Dj/xÎc?BÄì?ïþ7ŽC›1?DO:'F¶?,‡ÆLïâ?DO:'F¶?ïÔ~€Ä_?|Êòÿ™?uÀ¿ÿÏŸ?|Êòÿ—?ïû¤ÞûU?2­V¥ë"?Al‡˜ªì?2­V¥ën4FGL J2336.6+2356?ÖÑ1þ°ÀAê]yЦÀ:'ã8IªÀ<}\ã/å¡@sòvŽ+@‹4*©ø?À¬Ëxº?°Ö‡X¤\?ñ´)¸`.>@'#uP5¿ïø
ñâ?ïÿ*'Š‰[¿å3¢Câ-¿â•"z›¨¿×Ⴜ]hç¿é؃""^ŸAGNbcu3FGL J2336.5+2356B2 2334+23?ïö–Òjl?HØÛg¨´V?RÒ[+Ç(|?HØÛg¨´K?ïíݸ‰&?z×À<j¥?b"GvÙ÷x?z×À<j¨?ïÑ]QÊ?xLÓ>œr?wsvÑW*?xLÓ>œqþ?ï¤Cy£?vòtkßDÏ?†þ¯9a—?vòtkßDÌ4FGL J2336.6-4115?ïñRYêx¸ÀQHÙŽuyÀ9—ÇÜ£¦À<$«:«Í@Ã×öv"\@»tÝøn;?±dáVÀ{?½Y(ÿíOh@	Sü¡¦®U@zßøx¢¿µ+Pæ¢`è¿ÝA3¼pQ¿åO°!Etÿ¿æГ€ÐÊÞ¿åWõT«S¿åOß;AGNfsrq3FGL J2336.5-4116PKS 2333-415?ïþ¾ø\J?"1$ƒP
˜?$Àz;o1?"1$ƒPH?ïþ,‹ù?FÔ:í¿ÔQ?->G@o¸?FÔ:í¿ÔS?ï¨cë–"?ƒ™—Ü«¸?…ç8Ú[s?ƒ™—Ü«½?ïþºD{¡1?,ãIû?$[¸EíD?,ãJ94FGL J2336.9-5859?êÈm('¿œÀKÐ<³åuÀ;VÅÓ´G›À<Á ªšrÝ@/ª›õiy@¸™aeu¦?ÜÚ]-W§?Í·Ÿ©~+?çx˜˜Ú@X…ïBÃt¿ïª'ñ¶'!?îa«IQ¿å¡­>¼ÿ$¿ä¶+ÀÎð¿ïÿìêy…þ?î9æ@;YrAGNbcuPMN J2337-5901?ïêy?gÄÂÙa¼?eñ~]…Æ?gÄÂÙa¸?ïñw#óJ?yŒðöÐC?]¸kÄt?yŒðöÐ>?í¸m˳"œ?žF&GkýE?²<'¢cÛ-?žF&GkýG?ïñޏO?SŸý†jžZ?\BàÅaÖw?SŸý†jžZ4FGL J2338.0-0230¿ë‡öÁœþÀMàÐÜüŹÀ9/{T44»À<
ª}í@tÐ%Ǻ¿@¸t »ÌÊ?¬¾lô-u?«ж'L?üu`4=þ@yFCcA¿×Â;cÙCS¿ã6M½øô¿æTŒê^®¿çç¾Àš¿íäŠÄÀ§?ÆP²ŠMÈAGNfsrq3FGL J2338.1-0229PKS 2335-027?ïýÖZ ?*ªÝ"‹÷?1O=.þ?*ªÝ"ŒX?ïþw7ä?HÛª#®Z?/،ñ¼¤?HÛª#®C?ïÕKQÒtV?rÉbt‡ÛX?uZWÅÕ¾?rÉbt‡ÛZ?ïÿb+?Rᓱ˜í?îS¿šÉ ?Rᓱ™˜4FGL J2338.1+0325¿Þqn¢vqzÀKX³!ž¶À:ÁêÃê¦À<AF¹!õ@…F/9T@óMAÒ2g?ËmÖݜӶ?Æ	ÃbÀ¿x?ûI·ôÎs–@6+™Þ¿íÀ.ž£ï‰?îjA¢a¿8¿çöLÃ'1¿å{î|Iý¿á©Šrµ)B¿ïÿýç!éAGNagnPKS 2335+03?ï±Èº´xƒ?ˆ£ç¡Ïº?ƒÑRáß?ˆ£ç¡Ï¸?ïÝðvåN?†y2•šs&?qč|ØÅ?†y2•šs'?í®I¹ üE?¥¶AUöC?²²2øÖ?¥¶AUöA?ïWÊîµûŸ?†Zò ÑIÏ?•¢)@Œ;?†Zò ÑIÑ4FGL J2338.9+2124?èÍ4ÑùÞÀC2¹^Zÿ*À:»ö»³ À<UCh4œÀ@_FrÖ@(è6ú?´r4ûµB—¿‹v±ÚzÉ?Ø&IaÉ@(Çí?)?ïÿ¢âîwA¿à"-F<$¿än$Öyù¿ÞpDAùJ¿ÙK"\Ðg¿Ýô½ÑâAGNbll3FGL J2339.0+2122RX J2338.8+2124?ïþ•÷ۃ?#`~½Ï."?&®°'GÒH?#`~½Ï.Û?ïþ9qsF?PÁM[Žy?,hèÆ+¡P?PÁM[Žx?ïølúÎ?Odv°üÙý?NLÇòí?Odv°üÙº?ïùmŒ[×ô?8ò†.›;ò?JIΐ .?8ò†.›;Ð4FGL J2339.2-7403¿²¢÷Qì`ÀE7~ŽÒÀ:—âà4‰À<yyRژ@X*"~&Ì?þ¤(hÔÕ°?¶äø½–xþ?¦Õç}¨!r?ð˜í×ßO†@o[¸7"l?ïé`ŒÝŸ¿âÕÛN¿àÜ<ÁÒGá¿ÛOBŒf¿ãy«ó8qa¿×À
6Ih)AGNbll3FGL J2338.7-74011RXS J233919.8-740439?ïþºD­wÚ?Ö#•hÒ±?$[µ('U
?Ö#•hÒ«?ïþjÑrgR?D1tã4Ž?)RèيÜ?D1tã4¸?ïúÙTm.Œ?CFŒa'?Dš®KEϧ?CFŒaF?ïóª"
y?B-ÿJ¹Â?XªÙåÓò?B-ÿJ¹Á4FGL J2339.3-2656¿ØÞ9õàÀR}|o½'=À;oˆ"xÐÌÀ<Évú2`¥@í°°ŒzL@Wª¹|ð?Ïå5¤Q®s?Œ°'¿7á?¿ø¢~¶_@»©äÀ^?ïª9ú͑¿çôÉ_¿åÕ¾]ž@È¿Õß/»Y‡Ü¿äÉï•N±¿ïéõ!T¹kAGNbcuNVSS J233917-265638?ïÿmš'EÇ?ð>ĵ\?L»G<=?ð>ĵ0?ïþú"Ò~|?:Òð£0t? VÂØ5u?:Òð£0*?ïî=¡˜8?g¡·ÈÓK?a€Â^gȉ?g¡·ÈÓA?ïþí²É'?ún(O|½?!.TÓfõe?ún(O{4FGL J2339.6+0242¿Ü—gÕ#ƱÀKÀ"`ÑÀ:$رÝ]>À<+ÉMì@¡ÑÖvï¡@GPܑeî?ÃMK7`êQ?É¿?#€c@ù«ó8qa@
£E±,?ïܨAÓ	'¿å~Âþ—Ë
¿ç¡]]SBG¿èÉv7]d¿ïø[#*¿ïü'«@‹AGNbcu3FGL J2338.7+0251CRATES J233930+024420?ïåbƒ×¤ ?s©™¥JN?j|([à?s©™¥JP?ïé9šš?‡¼=e/3?fÆeçe÷R?‡¼=e/5?î{]À
ûÙ?šŠ†õ!¶?¨J#ÿPBP?šŠ†õ!´?ï_¢"¥"?5*˜£M ?"­‹Ml?5*˜£M 4FGL J2340.5+3854?Ы²Üy9À5ëVûW÷À:á½ñg·À<…üÉêš=@ Ih«»M?þó•:a%?Èîºu\N?©PÃß4к?äfg=%û<@1" k³?êÚÛé*Ñ¿ÇÀ[zO&"¿é´ò?øé`¿Ô°– ÀÕH¿Ï^c¸Œ¿êg%©ôçAGNbcu3FGL J2340.7+3847GALEXASC J234042.83+385510.7?ïúÌ¡Sî_?DŠ­˜?DÍz°F†?DŠ­À?ïýRيï?UP(žì†?5i3¯ a?UP(žì|?ïäS]—PÅ?lŽ¸¦[ª?k¬¢h¯:¿?lŽ¸¦[£?ïçp"Té?Sßád4+ô?hk«ãý?Sßád4+ï4FGL J2340.8+8015?좂^;=@1Ðx·¡Â]À8»ZôB\œÀ;œ—ü
§ú@ Øf3Í?ýmlš]
ø?¦/ºîí‰?·ø«wènê@Qš&‡S@uþÕ®Ë?ï¿t¿Å}M¿â¯LåÄ¿ÜÂ~_o׿ԈB#þÀ¿â\ʵ›X¿ÞR+[xv´AGNbll3FGL J2340.7+80161RXS J234051.4+801513?ï¿@Z¢Ü?€ú
×ýù¥?€=/éWHá?€ú
×ýù¦?â¤ÐÎílÀ?Öú¢U
Á«?Ú¶^b%&'?Öú¢U
Á«?î¼d¸×?œĚD"Ç?¤9¿ÄrŽõ?œĚD"È?ãΫ큵?³ëöwvë?Øcú¨$ü—?³ëöwvë4FGL J2341.8-2917¿Øže"fûÀR¡quŽ!–À:öä/À<±páêkC@~¯—ݬÄ@ۀ©Þ‹;?Ìs‹èÖî?Àx)Çόñ?ñàV·œ¹à?ü¢òÙPé§?î³àֆ¿Ó¬p¡RË¿ágž	jâÍ¿âBl¡"ãø¿ïÿF!!Ä?ïù‹a~ÖAGNrdgPKS 2338-295?ïîrV;€5?`åqõÍ?a©ÄÉ®?`åqõÊ?﮸±È.?'#<Xó'?"QӍÿ4W?'#<Xóƒ?ïzhª
?"9¶upëÙ?Ÿ0²ê¾NK?"9¶upëÙ?ïh¸p™{¦?"«'w¼õ.?'èñìЋI?"«'w¼õ.4FGL J2343.6+3438?ê/'¼ªs¬À:.o`àëhÀ:+'›O|À<>9E›ëƒ@ á{´×7µ?û=uâlv?º…™\‡ëF?°ZKÐãݵ?ö T3]û^@Lï‹h©b¿ïԍöÎ(?ê`=X¿ÂÝÚ%ÐÊ¿Öe
{"Ý¿ÞÝh»Ö/w¿ÅWÙc¯AGNbll3FGL J2343.7+34371RXS J234332.5+343957?ïÿ4»Jƒ?J~HËiU?hŸ–¯ín?J~HËiA?ïýJ_å'¨?VԔÅ\Ü?5­ÖÂÈé?VԔÅ\×?ïòÇC¦b³?cû§ÆóÞ·?Zqx³:œ?cû§ÆóÞ¹?ïôi}N?Ipè©$2&?W-ÇcüÖ?Ipè©$2	4FGL J2343.7-5624?î@ÂÒÀM(6CˆëÌÀ:Íã˜Á,†À< †TBw@Â>%Õ|Ÿ@ç<º›qá?ÀÊ¶Ú ¿–rŸj`h?Ôì¾Ü-"@Uf¤S1?¼æ+ÿžlx¿ç¶Â3얗¿éÌVè'¿Ô¼Ì¤ˆàå¿í=Û,áàZ¿ãYyMÉ·oAGNbcuPKS 2340-567?ïýԄd¦?)¡B6^
û?1[ÜÚÏL¯?)¡B6^?ïþx< @?DWA¦Ïm²?(|=û÷?DWA¦ÏmÂ?ï햃Úi©?g9Hðã¡?bi|%–Vý?g9Hðã¢?ïþñÓϟ?—=xý}¶? âÃ~æ?—=xý}4FGL J2343.9+0546?ïzéîƒâWÀJ¢pCßÀ:ª¶P‰…OÀ<iDo›™N@…Ã÷¼º@%`â˜ç?ē['÷
é?Ò­Ûzº†N@	»ž ç×@J¨;rò¼¿ëoyȸ?ѼB¦m½s¿ã
,kü¿Øò.Ü"¿éΕßе¿ïÿëÞ
òAGNbcu3FGL J2344.4+05491RXS J234354.4+054713?í7 ?¶´ïhŠ²S?·ŒÆGzü?¶´ïhŠ²S?íö@*CК?Ážå3?°Mþ­á{7?Ážå3?瘌`]?¶B×õî?ÑîÎç?ÝG?¶B×õî?ì¶açlÌ?¦"bˆ¤¡?ºLðęŸY?¦"bˆ¤¡4FGL J2345.2-1555¿î˜æ
¡4ÈÀQ¿j@»À7!–5dfÀ:þO'åJr@Þ_ùÎj@E}àÖo
?'àQ—ì}?ºW±þÑgø@&§lH'¶þ@ª#
¡S¿Ç¼€xá¿Ùòì;}·¿â_Ï=ÀTï¿â?êÁf½¿çø@îݘͿ糝쏋AGNFSRQ3FGL J2345.2-1554PMN J2345-1555?ïæ+×	D?dâ"íë"È?iïÔ(ö¼
?dâ"íë"Í?ïßÖµ÷L§?ƒÍÔë ?p¥Y¬+?ƒÍÔë ?ïKQ²Êƒ?"vyåëô?–•Í馯'?"vyåëô?ïâi>¥Þä?oà"Té?m–ÁZ!3?oà"Tî4FGL J2346.7+0705¿ÇÍ´Ó$ZNÀJ.XOLnnÀ9,¨hiuåÀ;Ð֟´eÎ@ 51¯=?ýŽ Ç‹Dl?­-=¿—ôÃ?–oBᄝg?ìHÆxõ@íÈs÷žˆ¿ïÿíUÙPi?ïþÝöÀ¼¿âðûµîcö¿Ñ	ç_u0"¿ã£—I]A$¿¾_ðÀòÎêAGNbll3FGL J2346.7+0705TXS 2344+068?ïýמ
ô?1–2,§Uê?1Cÿld?1–2,§V?ïûx"DÍ?bÓAô¼ë?B®ïÏ?bÓAô¼æ?ïÀd\âSY?Ž–H i?ÍюÖS?Ž–H l?ïÕA}»;?n—«øûÀÙ?u_A"br
?n—«øûÀÔ4FGL J2346.7+8008?èØÀ®6ƒ-@1 -à
À9º¶åÚºÌÀ;ÍÂ5fê@¦7Õ.p+@…³ƒO«9?»(
æª?ÂK²›s8‡@iS×@úȗ^¿ïÿÀ_V&Ó?ïÿHkÇÏ¿äçøé
¿å÷BÂo¢¿èy‹!0Ò0¿ïþõÎÇúAGNbllWN B2344.2+7951?ba4?¨vÌ#ùJÒ?¤>EyÙì¼?¨vÌ#ùJÓ?êgÛ¨¿?Îy¡Ÿ€n?Æaø']?Îy¡Ÿ€n?ì>Ÿ²å?­Ó5ENq?¾o ×?­Ó5ENq?éA"}ŒÐÙ?³¯"iÝ9D?Êûv	̼œ?³¯"iÝ9D4FGL J2347.0+5141?ïJñ=1c†À#Ԕ-IgÀ8* Á@§À;h$Ÿòy@EY,ìó?ûñ«#.Ù1?lÊ{QE?¢µê!
Uˆ@TÀ%@hbå}rÇ?ïÿ5À+SÁ¿ºcCÇ* ¿×j[h†|¿Úï ^Å2O¿à
͞ƒä&¿×*kÄR{AGNbll3FGL J2347.0+51421ES 2344+514?ïÿ%ï³ÜÆ?j¢Tt¬?B	"g0¢?j¢Ttb?ïû']Oë?W[úÖ-()?CÃbŠÀPË?W[úÖ-('?ïǑA€³=?º{(›?|7_?¦`õ?º{(œ?ïè7ÏM?V¿Un]¾?gÈ0ñë±Ó?V¿Un]½4FGL J2347.9+5436?é'ÂŽËÀlÀƒ#5.À::sí7¦_À<4¨ÒÁ'@!†Š!×k?ù?yB=K?¾%ŸÌ¹–?È'?Š¤z@ÁvÂÔüF@RbŸ\|-¿ïÿéÅ+Ü?ï÷‰8ùEÒ?ꝡ»üñ¿ÔŸ4£ ®Œ¿×ՙd•€Û¿×n:%âeAGNbcu3FGL J2347.9+5436NVSS J234753+543627?ï¾`ùz°?€21HùsR?€gÁº¡T!?€21HùsP?ïÅÕt³? ¥™W£Y?}r•pŦ? ¥™W£Z?îÎÞu·´?š±ÑÎ=×?£'¤"¯?š±ÑÎ=Ø?¶M$?–·tu:?§tžt›-Í?–·tu94FGL J2348.0-1630¿íBg‡ïŠàÀQù2‹m†ìÀ82Îí8}À;]«›úœê@ݾ•Q‹c@QþÍ?¹? ãò¿`ä­?­H­Bî½
@T¿Z'È@Ïîq¸)'¿ÊÊ«õ¼°¿à.‡'?àÁ¿å&ŸÔœ$¿äì~ÃÕW¿è%Ë5ó×Ô¿é™ÝŒ7±AGNfsrq3FGL J2348.0-1630PKS 2345-16?ïûR'8Mx?@‡%®'äz?Bµ÷Ê!Õ?@‡%®'ä?ïüðk"ºW?M°•b&/å?8|£Ú-:/?M°•b&/í?ï¹£&ò¤?8:5Ç?—6C~?8:5Ç?ïÿÎбÅã>ñ™—êÁÊ>ø—§uK>ñ™—êÁ
Á4FGL J2348.1-4934?í
*ÝcJÀPlvJßøÀ;,ägô À<¨¦¹<Í@‹>âéÅ?ý‡RÀ—4?ÞKþzÄÂ?åՏHÝ¿c@úÆ[¯S@	M/ê©V¦¿éf™£U¿äÀóEšN¿ånç´¯ ¿íc¯!–'Ê¿ïý³¿µ?ïûžaTƒ»AGNbcuPKS 2346-498?ïþϑ¥Á?FJ›äTB?/3å£Ù‰?FJ›äT.?ïöØy¯'?nQZ631M?SO Ý¬?nQZ631Q?îâJLä?•u"qØ?¡Û[1¿Þä?•u"qØ?ïðØö*?[Eôˆs?^Nßõª¼?[Eôˆs4FGL J2348.3-6049¿Û"P{4VÀKT¼M"ÉÀ;¼ZÔ–À=»µMTG@lR
¾Ú?ùžõ#-+²?ÞTñÿŒ<º?ÜÊ¡yaë­?ùã÷aËÍ@氛"Äÿã\ܯ˜ß_¿íQ±k뿸4Àüßå¿áõN€ìy¿àÓnÝ-m!¿ïÿ:=°AGNbcuPKS 2345-611?ïóÄö¯è?Z¤ÇÌÑT?Xv /˜?Z¤ÇÌÑS?ïýxëGÇÕ?TkŽVAÁö?48¥ÁÁRŽ?TkŽVAÁê?ï&>R¼?"å\@9(?›<5¨'?"å\@9'?ï÷yÀ'.)?Eتhi?Q±£®??Eتhi4FGL J2349.2+4535?ÿ1
Ì×+À/ÒmÚÎîÀ:¥ub'¬À<
È°ÞZ@—"Òã]@"Âqÿø?°yÅhÕW?²öwÁ½o?ñ/N6ĸ+@
ªúý·¦J¿Ðõ"¡•'w¿áþ˜h¿äÊæ¾:Å¿âz?+Žú¿Õ£'{šÖ¿ïÿX¥³ƒPAGNbcuTXS 2346+453?ïÿ
iζÖ?k•¡^	þ?²Æ)%^Ù?k•¡^	Í?ïþ¯Áô€Ô?Aw¤·B?%à·ò³?Aw¤·R?ïöùÒY¶^?T÷Ý Ù?R[L"D¿?T÷Ý Ê?ïþ¾Ô_—Ó?Ìpt0ú?$º'ÐK?Ìpt1h4FGL J2349.4+0534¿ÈN)OõÀKo?Rü&À:`%t-ÏFÀ<KÏå†6@¡-g—>@ÕÓ;{×?¼ÿØè¹èD¿"©*±.‹¯?Ö%Â1hWØ@	â²r®?ïV%;"뽿éàp]‹ …¿ãßvó|d¿æwÿëÞ
¿ç…æ>7ô
¿ïÿÓ?,» AGNfsrqTXS 2346+052?ïþ;ÿs?+LÁ	ÍȄ?/@¸Ø­?+LÁ	ÍÈM?ïþÄ팞?FŠˆ7œïó?(±'6?FŠˆ7œïð?ïãf¶ø3?o
¦•÷U?l™=Ì?o
¦•÷P?ïú¸å$?2z˜Ä/4?EœkoôH?2z˜Ä/3ò4FGL J2350.6-3005¿Û¶(ª-ÊÀSA5Tu£À:#5'Ì÷À<k‰öŽg6@ÙZÂC[õ?ÿÅ%Ù®\Ÿ?¹U%¡OE? ¯&ɘdæ?ç?–¹‰$@\ü؃9[¿éµ³áC|W¿ßè|U»ô7¿ã×jµ€€¿Ù½Ü¡u0¿âf˱CÚJ¿Û²Ø
€ÇAGNbll3FGL J2350.4-3004LEDA 3231681?ïÿo˼?O´øÈ[+?'ŸÈ‰v?O´øÈZË?ïþ˜z ¶¾?H9d­¯?&x]ô"	?H9d­Ð?ïø>t$†?bü•"tLY?O/oÑì«?bü•"tLX?ïþàžNûQ?^µÛã&'?!öJÍ¿?^µÛã%'4FGL J2350.9-1416¿ïý²"/ZÀQ»y(àÉÚÀ;lmî$nÀ<ÉÎ	îü@]šÖZ•"?û6*^x[[?἖S"ûË?ÜH$".q?ù/H!×Á@~DÖHÌ¿ïÏBÈÒlI?ïòX!ªÍ¿ÛïY—Œ¿á\à
—2·¿â ¾z#³¿ïÿ>9 ²þAGNbcuNVSS J235111-141557?ïíÝ¥½Oy?dI·•…ë(?b"ZB°…Ñ?dI·•…ë%?ïîõo='?~G'Ö'6u?aí
Âُ?~G'Ö'6q?=S(Ø?œ&ڥۆÚ?¦Œ*Írƒ?œ&ڥۆ×?k–?€ònòûf?‰ù'¥;§?€ònòûf4FGL J2351.3-7559?ïYŽÄu^ÀDJ­ÕÀ­À:G,å;YÀ<d»±òUó@ iÐ~25?üµY~ —O?¸É­6Ú]?» ç¬!0§@HIёX@ØÔ2Ü?îöúÓpTý¿â¸§z¡‡¿ÑQÐb©~¿Þџše¿áú@¨f¼¿áz螺jÊAGNbll3FGL J2351.9-7601SUMSS J235115-760012?ïÿÕ)Ò?u5Pïû¶?EZŵ?u5Pïûä?ïüG¨Ch?UuûVÕ?3?=½çd²ä?UuûVÕ?,?ïóÞåØ?d7A¥yO?XCóø4LÏ?d7A¥y6?ïÎ¥Y?dʔSDò?xô-Suz??dʔSDî4FGL J2352.0+1750¿ï¢ò'w ÀEd9¼º0À:¤Ó‰pÀ<\Ti
à"@T6üÁ\+?ÿ:F"bH?¼'uÆ«¡?ÀÚ™Z"†@gMú^ÖO@DVä"=	¿æK¿[o'¿áK+­,ôU¿à'ÉEnŸ¿ÚwPCKã¿éø@îݙ¿è,ì\µ½AGNbll3FGL J2352.0+1752CLASS J2352+1749?ïø؋'¼?Jšˆäâ?LÑ»ý$?Jšˆäî?ïü¿šLdÝ?SڍäSÊ?:-œÙÃ?SڍäSÏ?ﺄJ0E?ƒÙüÛ)Ç?^í`3ï?ƒÙüÛ)Æ?ïò·î†¸ø?L4mÔ3;î?Z"òŽû?L4mÔ3;Ù4FGL J2352.9+3031?¼ŸºAºÆ°À>®˜¹ZÀ;RƒZ'ôÀ<‡˜(€QÊ@¿§·¿tu@íx:¤?·Êóìn~¿¾\€^Š$@…ƒb°@È>¸w€??ïPz¼¿çwåê«%¿ä´þ¤á ¿ä0]ºpT¿è{~@w¿T¿ðAGNbcuMG3 J235254+3030?ïûL«íŠQ?Bq6XÜ?BÍPIÖ¿"?Bq6Xí?ïÁ¢n\Ü? ¦ÐÙô–?.ÈÑð? ¦ÐÙô–?ïyRÒ>"œ?v†*ô?Õ¥¸-Œp?v†*÷?ï~À·ÖH?| ¾´Åè?'é<W	?| ¾´Åê4FGL J2353.1-4806?çxꔍtÐÀP‰VC´À:ÉÝÑôÀ<Å
?#@L£Ór¦@$É Èb?ô2â€hE?Á>Áh¼,?ü\e¬,CU@Oš"Ñ
Ÿ?ìÕ©ë të?·˜Jd°¿âzé«)äÖ¿Ü|Tú®1¿å`ºŠªéM¿âB¨@ÑVtAGNbcu3FGL J2353.3-48052MASS J23531112-4806045?ïÚÖmÌrù?r|}3+ßM?r"ÉƄ)?r|}3+ßJ?ïôè[­Ô‡?pGÓÍg^?V/H¤Vó:?pGÓÍg\?ïÔ¼Ššxè?w¢²"s­?u¡º²Ã‹ö?w¢²"s«?ﺕ^_ý€?kaøœq2·?Z¨h ;?kaøœq2º4FGL J2353.5+6646¿à½",mÉ©@&QßƤ•À9ëîÑÀ;'F1<¸î@½¡†øØ@õçB™Ø"?ÇéÀãàd¯?§ðd+´Ë?ã—cßM'ë@Áûa4Î>?ïþùÛ"Ðå¿Ùÿ€>Sοí5{!‰g¿ã^«‡ça¿é ÝZ¹‰ú¿Ô6ŽûçAGNbcu3FGL J2353.3+6639NVSS J235301+664243?í°'WTz ?´Ó2»ݨ?²{uE\*ÿ?´Ó2»ݨ?îºéÎõî5?»;=FúŸf?¤Qc¡¬?»;=FúŸf?êñáɊ?­ƒÃÚ?Ä8xÙ×»÷?­ƒÃÚ?î"QÙKyt?'.oR­M÷?§ºâkHh¾?'.oR­Mù4FGL J2353.5-1457¿ïÉœÏ÷çÀQö¨~8ëÀ;DâΖÑhÀ<Ÿþ­©@ (&VÉ@íÅjؼ?ŧRiÚ9G¿­eyxù?çþ)f*×D@÷»õ9'"?ïîX¾7,¿áËހ("Y¿êà*b)?ê¿Þ"aùð†¿¹ n†,¿ïÿÀéz-AGNbll1REX J235320-1458.9?ïüjw­…ì?:t0m´ŒR?<¬B"Ш^?:t0m´Œ[?ïüc…Mþm?Uí¶b3?<ãՐ ë?Uí¶b>?ï×z¡\±?vC²§WPç?tB¯Q§xG?vC²§WPß?ïôí¤¹¹W?M÷bªI?V$¶ŒRÆ?M÷bªQ4FGL J2353.7-3037?µj"ÀS9Ϫ͞"À:7\óöÝBÀ<}:Y˜!Ê@ÇO"L«T@©3]$žE?¿¬Ð6f?¶a·U\ä?ö,û
͹\@¤Žèe¯‡?ï¦Á4éÙ¿ä?£ƒþ'¿Þx¹d»•¿à¡åÎ%'a¿êºM8—÷¿á4ÂkñAGNbll3FGL J2353.6-3037PKS 2351-309?ï«+âqÂß?€UJ;	?…5cH9?€UJ;	?ïç•Ð÷¾O?z'cÖ`NÕ?hj/A¯€?z'cÖ`NÕ?ï
ªkTï?"^"/?žJ²Žb?"^"/?ï€2—ƒsc?z]¨Á46'?óZ#'?z]¨Á46"4FGL J2353.8-3911?¼#0³'ïÀR?Až0PÀ;	æ~OÀ<Á|Ôfõ@ …±…@ïó»NH?ÑbäRzv?ÅVV"÷Q?óœ}YÇò@Æí­B?íü݀ú}¿é$â7˜¿ä=а‡é¿å^à
AL¿è5é
†¦¿ïÿþBe«+AGNbcu3FGL J2353.7-3911NVSS J235342-391442?ïõ²Åø??XñÊ«`þÚ?Tšũ{?XñÊ«`þâ?ïîÖóýsç?s¼TÓb?a)Œâ?s¼TÓ_?ïbÌ5èù?=âYK)?"¼æyBàë?=âYK'?ïLjÂ<€k?g	92ŠÚ?|;žá¿Ê™?g	92ŠÚ4FGL J2354.1+2720?æè*®KÀ@çu¸eÀ:ÖƞµbMÀ<›
ü³Df@x>He"@Òµþ,Á?ːßò?À)á¹mõ?ô}_Üßiˆ?ù§õ
j¿Ü°h}—ÛS¿á»'Á^Á¿æÒ<çè¿Æ6`y½[@¿îƒÏBrì1¿ïÿî' ÇAGNbll3FGL J2354.0+2722NVSS J235402+272328?ïø%ڊ¶Ô?M\1ëͽe?Oh•Õ$´?M\1ëͽq?ï–O/¸_x?¤Áõè4?Šl4è!ö?¤Áõè4?ï¢CäÞh?…D·ÜÃño?‡oÿf?…D·ÜÃñp?îÍØ}.¶?'ÝquOó?£"x-ŸŠ?'ÝquOô4FGL J2354.1-0958?réŠ{ÀQ
Ÿ¸fäÀ; ïܸÓÀ<|ùûA@ŸXŽâ[@²c"úÎ?Ða؂b›V?¼_õÞéÛ?íï8œÿ¨@Ý›ëÙW?î®X£/D'¿èÍ_ߎ›d¿æÆuÐfµA¿ØxÕÔ³K¿ë{¢´¿ïþaå£2AGNfsrqPMN J2354-0957?ïýÝÎöß?6¤;¿c_J?1¡ˆI	°?6¤;¿c_?ïós2|Õ?pÜØù_ž?YϛYÇ?pÜØù_ž?ïÖÉÅ7b?xŠræJ]?t›qdN)?xŠræJ]?ï荿ËQ©?Xn;@Ör?gr@4®V?Xn;@Öu4FGL J2354.6+4554?í¬l\ò8À/¬ÚQÎÀ:¤l™†NcÀ<pÈÜ}Cø@2êm·A@=Û?VW?È)Eßaô?Òð ÿê[@1o† ˜'?îo\k«¿íh­aÍz?ïÔÊ\°?¿åã$\֚¬¿çèŸ8iÿ¿àoUB§šc¿ïþÍ?äF'AGNfsrq3FGL J2354.1+46054C +45.51?ï'º&äÞ?©Ûd]Ý»?ŸÍÈ»#dA?©Ûd]Ý»?æ³Y×I?Ôå¾DºX¾?Ó™LQmÆ?Ôå¾DºX¾?é1€49¾c?³{ø|ŽÓ?Ë9ÿ/t?³{ø|ŽÓž?ÓØäÓøØø?¹åI–Û?捖""?¹åI–Û4FGL J2354.9+8151?½0‹Ì‹@39¸ºÇËÀ:*Ô2ò›"À<B€'،@D5݇…@ÝÊeê?¤?À.I¼ât?¶y<×Ì°?òF>¢‹±@®õt‹Ã¿Ð-lŸ»q±¿æHdˆ?Õ¿æ=ò^¬³¨¿è–6—k¿ëpù'7}E¿¸—ß/OúAGNfsrq3FGL J2355.5+8154S5 2353+81?ïÌ,T+é?uG4âðá¦?yéÕê8K?uG4âðá¦?ï逰ª`²?ƒÂZBÏD?fOUŸNý?ƒÂZBÏE?'"5Ó?‰–Yêˆ?ŽTwr‹?‰–Yê‹?ï'âi!?uHȟ?‹¾Gxe·i?uHȟ4FGL J2355.7-3351?ï3¤Ýd-ÀSzž+ϒÀ:,ÊëK=À<™QþÐU@wnåhz@€öÍ0 ?µŸÍ»4I?Ÿ¼*¤T™Æ?ãa¬ÃB	@õÕt'!{¿Åì]÷,è¿æ*—MŽÿ¿æq?2oê¿çäû¨'k¿å#'@ßÄ ¿ïéþ¡[.ûAGNbcuNVSS J235538-335225?ïÿ:ŠC}´?}!Ïښ°?®·IlÅ?}!Ïښj?ïü«"wî]?U
ÊM¶Ch?:£\@ú?U
ÊM¶Ce?ï쌯ih?elØ,öˆ?csP–˜£?elØ,ö€?ïúáìðé?7t¾X¤P?DxL<[«,?7t¾X¤4FGL J2356.2+4036?Ìd]pÅÀ52¹¯æÀ:"ØÛÎÈPÀ<Z¾ÎÝHE@ =û¹tUg?þْx=(?·0t¼ëXS?ª\Šo…?ՆŸ Âg@ͅþ‡/	¿ï¡ºÃ.¾?ÿ (¿ã'! 
ҿٛÈ]|\ó¿â"c'0qb¿×ïHÂçp½AGNbll3FGL J2356.0+4037NVSS J235612+403648?ïöú¸ö·)?K6­ßüï?R
Ž'²¨?K6­ßüÞ?ïúˆDè/{?_.ҕ|Ù~?EÞì_BÝ?_.ҕ|ل?ïÝ<¸@\|?s78*/¢[?qa£ßÑÁ…?s78*/¢_?ï³÷bÞê?tÆr÷/?ƒ'ÈEP?tÆr÷-4FGL J2357.0-4840?Ìó©(–ðFÀP:ÎÄÀ:ꋨ?OÀ<È«Yµ}ü@—Ì±Éç?ÿ¸j1Í?ÅÑH#w)?ÁèN2'úC?ûq¹_ã•?úý¿é+ÿbKO¿ÝŸæ+]Ò¿ãµ…Q8¿ã"ñ10#´¿ÚNÖ½;ŠE¿ïÿÚ
¢ñ1AGNbcuPKS 2354-489?ïò™tc˜ú?Z˕Ñ|=Ô?ZÍ8Î
?Z˕Ñ|=Î?ïÎëä
!¢?‰BªfŸa?xŠ
ùo.x?‰BªfŸa?諾î΄e?''rãù?†˜"L^æÊ?''rãù?ïhSdçúu?{Ñ÷½ÈV?'õ"c±v?{Ñ÷½ÈV4FGL J2357.4-0152?è|p+®;ÀÀNÏÝ~Ë·úÀ:z–ê'°qÀ<zô/è%@LN†öª@ñ*_Oð?ʪ¾ZO?´‹õÈ|Ü?ñ"4 ½@;ª%-?½¤Òݲù¿å_×5ÜZß¿àHBY@ãö¿è6±•+v¿è‹D× ef¿ïî¤"‰—ÄAGNbll3FGL J2357.3-0150PKS 2354-021?ï÷Üá0?Pe>‡§²n?PxÆ=õ >?Pe>‡§²l?ïþCb•C?B0¨®×6?+ÉÞ6«Í‡?B0¨®×I?ïÄK0Ö?€BTê|i£?}öÚg"öÇ?€BTê|i§?ïòž¯…ºF?I'·»dJ?Z ô‹qÐ?I'·»dJ4FGL J2357.4-1718?ç—%åñHÀRˆÂß
A1À:;<ó¦UÀ<C³aÁ»ø@ ãÍJ 4©?úü´=Š?¿ÜhKBôq?©÷#́?îmÓ­'ž#?ù ¤äüD?ïÝÍ:°Õö¿ë>³>±@ª¿Ø}[À›<¿Åó.ö¸ƒ•¿Ýþ‰Þ:³Z¿Ö›V½ÑÝ-AGNbll3FGL J2357.4-1716RBS 2066?ïüÑW œß?1¾@…)"?9uFûý?1¾@…)y?ïß ýR
??…)†hÊ]?p/Vùa'?…)†hÊ\?ïèÎý3JR?nÇ5 \Æ?g1̵®ƒ?nÇ5 \Å?ï'kmÕÝ,?x#!iE?‹e$Šˆµ5?x#!iG4FGL J2357.8-5311?îþ8Ž¹ÀO
LÂPrÀ9³v/1EóÀ<B­Vœ@œÂ†!í'@…	¿œ?°1¶±W{g?"°Y_ÓáO?ߨ8ã÷5×@¨(#µ'È¿ÔDx $ο槹ž¿çK|€.8£¿æšD¿ë^œ£9UŒ¿ïÿëJwAGNfsrq3FGL J2357.8-5310PKS 2355-534?ïÿ…"Iö€?=m‹BÈ@?·m'`<X?=m‹BÅC?ïþݘñÆh?<ÌWD	ÿ³?"&p㙍Ê?<ÌWD	ÿ¼?ïêÑoy>¹?d6é·'?e.†ÁFN?d6é·k?ïÿï´dÉÔ>؉¢ÑÌãˆ>àK›6,Ûç>؉¢ÑÌä«4FGL J2358.0-4601¿×f%ôêƒ&ÀQÇ%ÃßÀ:UŽ7£À<›£í°r#@üaŽQ@Õ8ü Ïï?¶Ml€—ü¿ !`!þ­p?ä)šÞh*·@f÷1OXX¿Ý§dŽu¿ä³[wN¿êeøí½]¿â¨¯à-¿áîKØE¦Ó¿ïÿ¢­>'AGNbcu3FGL J2358.0-4552PKS 2355-461?ïþÖÐò7?"ZùBéÃ,?"'ð܆ùš?"ZùBéÃ??ïþócXö?>ö†oÔÜ©? ÏéÊpˆï?>ö†oÔ܁?ïçaÓ²G?iQ¶poÿ?hž,M÷¸™?iQ¶poû?ïÿ{.¤í?úÚ¨d¯m?pš+beE?úÚ¨d¯{4FGL J2358.1-2853¿èpš}JÂÀS‡óõ"À:dü'¶vIÀ<œBÇû¬´@ŸpÕ*>m@ žÛøº?Àv†š
‡Ó?Âø » ýÑ@}¡›Æš"?þYÖ)ÂÇ?؉хCKY?ꫦ!r™¿ç49ÀGƒ¿ÛÎó£PQ§¿ïÿ½_œr½?è[¨«AGNbcu3FGL J2358.3-2853PMN J2358-2853?î8ŸÆW"?­÷û°åv?¬všÆÓ?­÷û°åv?î·oí°?³ËönQA†?¤É/Dø?³ËönQA†?î0!š+m?œ¸n¤Ià?¬ýïv]I-?œ¸n¤IÞ?í|ÿpç_U?£"-Ý6?´xÅ_?£"-Ý64FGL J2358.3-1021¿Úƒcȍ€ÀQE/Ÿ¾wÀ9Q}˜²
À<,ÄFŽ@jÉۀĶ@å:Ü?¯ÁðOÞº‹?µ\â?`ú'?þž"_¦XÅ@­Ô3É[(¿×Ų'¸#È¿ãðÝî]@M¿éR0^—ÿ¿ç2çHy–¿ìd¾ÆyÌ¿ÚäVÁ­´ÚAGNfsrq3FGL J2358.2-1022PKS 2355-106?ïþmÉÎñð?#г%?)#cà÷ž?#гË?ïý›ü'8?O**ðÄb?3 ;îDd?O**ðÄX?ïØ«¯M?ouf—\<Ï?sª(|uXÊ?ouf—\<ç?ïÿ$QC?¯F¥š?®[u×؎?¯F¤ÿ4FGL J2358.3+3830?ÁH>*{UfÀ72"áÉ´À: ôX,À<HÜ}Cø}@®Ö€Õ¨i@R:¸b²?»hŠØáƒ?'-c÷‡qµ?ÅŒ:
'Ö@
™dôÌE=?ïd' ÷¿ÙLo"È&J¿æ#׶ÿ†¿á'‡N={¿ÛMh=¬¿ê#¹B¬LûAGNbll3FGL J2358.5+3827B3 2355+382?ïü'!:M°?3š—'úØ·?;îö-'…½?3š—'úØÜ?ïþ¥ûØ0?CêúxØ?% N|äì?CêúxÞ?ïðV¾ýs?ho‰¿±\?_ÛR'<?ho‰¿±~?ïü"ã€ã?,­±ã#'—??Ó`ãøä?,­±ã#'ù4FGL J2358.5-1808¿ê¿Î™þÀR·D»ó¡À9Ø<Ç0«™À<<4ÿ¼
b@mS[?ýЋö–Ë?¸Š×´ÝAå?«à©^Ä£?õy²X­@@@tÁï•?ïä‹?Ž¶<?ÁK°B'—Ê¿àÞ¬É!F¢¿ÕçÓäC6¿ßMJ 4¨Ô¿åÎAvÂÔüAGNbll3FGL J2358.6-18091RXS J235836.3-180701?ïüüãä9¤?0dR?8àÞ2ãã?0dR+?ïýWõÍ$œ?NRšD?E?5@Q–Û R?NRšD?]?ïí-çÕ?m×°…©i?bÒìù*Ç?m×°…©w?ïèŒkÅå}?X ÑðD)9?gs":'y?X ÑðD),4FGL J2359.0+3922?ÝeôC5¸NÀ6cÓ^·E|À:bylÓgòÀ<7g0Â@Â	O_@é~¿\¢?¿y$?`¤A¿'Å˞?ÑB>éÊ´@
M|'¹Ø¿âïãÂwß¿çѓÛêw¿âÄ´š¦ßÓ¿æ*Ac¿Þï2²¾.¿ðAGNfsrq3FGL J2358.9+3926B2 2356+39?ïþ h~f
?(­WŒN²?-ùxŸ'Ä?(­WŒN±Æ?ïþÌÔÍö?A0'¨G£?#2³.˜]?A0'¨G£?ïá
?~.?q(†eØÈÂ?nõÀþÒ?q(†eØÈ·?ïÿ–y¿"?KâÚåï?-0È
h ?KâÚåW4FGL J2359.0-3038?ï֨Ҋ²ÀSŒSâÖÀ9ô·ˆ—é–À<;'&¶M/@ o"üT?üÈÄ3¡?´ ëóX§·?'«¥''"v?ßµ<ã5D@œåT-)?ïþé+0/¿ã'[ßú¦û¿Üôú¸îI¿Ô="_ÑKã¿ßQÞú¡Ç;¿Ó·'¸¬"XAGNbll3FGL J2359.3-3038H 2356-309?ïþb7šþe?%«ýÌ'Ä?)܆P½ì?%«ý̃T?ïý&öœP?MFMŽÏ1­?6ÈK{ë?MFMŽÏ1°?ïì­#?S_?kRbìiC?cRÜÀ¬¡Â?kRbìiC?ïðh}+›B?P6×#psP?_/¨É~?P6×#psW4FGL J2359.1+1719?ÑR#«ã
–ÀEâà"&þÀ;5áAÎ×iÀ<µÿÚ$@À€ŠÔÚ¸?þfv÷®!ç?Ë©…ïm·?ÅGФÕN?úÀâ³¾ß@¾ivf9¿ë‰¤>8Ió?ïìl5ç¿Ë7dpB¿å^"ñ¿×h@zi¿åƝ]É^ÙAGNbcuNVSS J235901+171926?ïì×ÅÚe?dh3à¸?c(ð:%™­?dh3à¸?ïùA>çÁ£?m†Ò@›'È?Jû`ùqÎ?m†Ò@›'Ï?ïgÀ."¶Ò?n?,Äåv?"ú;©%¨?n?,Äåp?ïÉ=Æ0(?gÿC?Ð#¸?{a7œçëå?gÿC?Ð#¸4FGL J2359.2-3134¿àîėËËÅÀSsC¬ÄðÀ:Ê§XžþÀ<Œ5¶›2 @üЁ¸&x@¯¿%D]'?¾šòŠ ªÅ?£ÿk@Ñè|?â%Ûüëx‰@ÌÆ+$q¿±=´€û"	¿ãB©D1ˆ¿ê-b
ç¿æAµaÌ"Ù¿éKŸÀûs¿ïü{Eñ{ÙAGNfsrqPKS 2357-318?ïþã¥Åf?
x6‰¾§?!Å®s©˜F?
x6‰¿?ïÿ9'íûa?6¸aS§èJ?Í¢@"Ÿ?6¸aS§è€?ïܚNÿM?rÓ+n¹?q²Ø±Y?rÓ+n½?ïÿÉ]Ú>ó2û3'>ûwQ¡>ó2û3"Å4FGL J2359.3+0215¿íóâȅOÀM<ÿdύÀ;b:	ç
À<´a‹·@ ëþ±Ì@`?ù·ãÑÌ?Ó˛ÿûMi?Û—ßÛq@ó‡œAÇ@ÏÅwÃÜ?ïÝH°rùó¿ïÿóÀ¬ƒ?ïÿ¤Á	¿×¾?kOÚ3¿àÞ¾fØ|¿æzD5ëAGNbcu1RXS J235916.9+021505?ïüC|IÄ¥?=ŸlœÎ?=ä±ÚÍ?=ŸlœÑ?ïüšØ2%?XÆY)ê?;/	>nÙÊ?XÆY)ì?ï«4Õõ>Ù?ðû§ýñl?…2ʂ°I ?ðû§ýñb?ï¯ÎrÈY?}ãB\my?"cM麡?}ãB\my4FGL J2359.3-2049?ž¹
7ȗÀS"¾7ޓŸÀ:Z€U$õƒÀ<‹³¢,@U¼!É(@øУñâ0?·ç
¶<h¿›€ØúÏáÍ?ä6wÁ½o@8¶Ñ"¿Û¯©ü=RÇ¿æ‰RÄÈòM¿âR°Ü¬=á¿Ý¡z¹"œ¿Üß!c'Å¿ÞÎÙAzHÆAGNbll3FGL J2359.5-2052TXS 2356-210?ïòڂê×?Rhø®é1?ZJú+ÆQ'?Rhø®é1!?ïý>8(j²?Pe‡'	?6>¼ªoi?Pe‡'?ïí\ÙQî?nûÐÉ`*Â?b£&®ä€?nûÐÉ`*Ã?ïøÊR~'?>8¾´DÄó?LÖ¶¹
?>8¾´DÅ4FGL J2359.9-3736?ïàË[uÀRºÛŸ'xÀ:òêÏS)À<ËR—|ˆè@8¦ÿ´?þ'5deÛ&?ÇrÀF׀?Т‰bñO@Ô×ãD8?ÿ‹O™Æ:7?ßð̆Uï÷?í\૦âW¿ÚdéÄTXG¿àJãq*¿éÓYG™ó¿×¸4½¤¼AGNbcu3FGL J0000.2-3738NVSS J000008-373819?îO䶴
Ü?«}ÛYé$?«´"¿"K?«}ÛYé#?îòËçN"G?°Ïí]Ú7? ÓA‹ˎ?°Ïí]Ú6?êëJ½ë?«6úÆ¡?ÄRÕQÃÂ?«6úÆ¡?ììJÚôQ$?¥žì7۝è?¸©(]vÒ?¥žì7۝è4FGL J0002.8+6217¿ÞÒ¼çK÷¿ª!gâE­À8Áœ©'žÀ;^`¯m@u@Ý®Éü¹@‰øÜö¼?®'‹`òË?Übþ<†n@%C1T??ü±åÃhÊð?Áºg"ôq¿Æ|Í[g¿á©c;8»¿çBëØ*Îá¿ïFMä¬g¿ïÿÌ~sM€PSRPSR3FGL J0002.6+6218PSR J0002+6216?.æ/Æí? |!ÑKÊ?ïþŸ=Ÿ? |!ÑKÊ?d±or‹®?sýj}¡)?ïëNtS?sýj}¡)?'¥¥2ð˜S?Y"4÷ÀôÉ?ïµik4=?Y"4÷ÀôÏ>ùàä>>ŠT>ð0@n‰¸F?ïÿÌ>7ƒ'>ð0@n‰¸F4FGL J0007.0+7303?î¼,wN|@$ìaR*o?À5'c;8»2À:xM'Ðÿa@.!|Òc?ý¯Qvëè?€"'—s¤'?ÑøÁ²½W@QTeâXO?ú$¸÷WåÅ¿ I[=¾QŠ¿É)ùù€´ñ¿Øör¸"@l¿àÏ>šõ9¿êˆ6šÆÀC¿î³'#iPSRPSR3FGL J0007.0+7302PSR J0007+7303?ki$cXÀæ?fjÕH?ïä–Ûœ§A?fjÕH?FÀúpé¾¾?g¹ýÀ£:?ïúOÁcŐ?g¹ýÀ£:?šâiARì?™¬ùH™:?ï(ì·eõh?™¬ùH™:?ð4FGL J0023.4+0920¿»,'wÀJrÁÁÖυÀ9›íQx™À<0j÷ŞÛ@…K2Åz?þ+O¤ƒ¨?¼J/¼P?ݞ7@.@¼æ")Æ@½f'|F¿æ‡Y%5C¯¿»,y@ïņ¿Ý‹ßœ³)Ž¿èqÊÛ[¿ëbœ!´/È¿ïû¾½?'PSRPSR3FGL J0023.4+0923PSR J0023+0923?wH=v÷bÕ?€#(
÷?ïÑo…:?€#(
ø?˜I~Ö?={?ª½›LvÝI?ï=´	N?ª½›LvÝJ?'¶	‹–*?…d¼Ìª\ ?ïrO³¤O?…d¼Ìª\?˜–¤˜2µ?‰Ã!é±ó?ï;JÛ>o?‰Ã!é±ó4FGL J0030.4+0451?ïú{yXôÀLÎi­BÃÊÀ7‹…º¿"À;‡^@'7|@Vÿë]0³?ü"µ—&"?š¶‡øºm?ÜzRõñ@?þº{'pÖ@¸wù
îF¿­@}Ú²z¿»Æ¤i¬A¿ÛŸv¼Ï)¿çŠ©Üݼ¿ît‰u_(¿ïþQ>¶ôôPSRPSR3FGL J0030.4+0451PSR J0030+0451?² µ=Å;?È
ŸÄ!=?í«éX\çY?È
ŸÄ!=?}ցïÁ~Å?ƒqXb?ïÄRü }?ƒqXb?ªc´šyqÍ? Ô'"ó"²?îYĶXhâ? Ô'"ó"°=qþX‰Øž=Kß!)ü	?ïÿÿÿÿÜ=Kß!,õ4FGL J0034.3-0534¿—b£®´AgÀQ³g ù	À8™¸Øú¹À<øä@bFg'A?ÿÕGª¹|Ž?¥=mbÈÂ?ÍیÙÝ@%Û°_®¼A?ûåÛÏI(é?¤7ÈÄ)¿Ô5Ñ>B¿áõ6þ™Îs¿æ^92¿í=¶y¤0Ì¿ïþ×@ÄnPSRPSR3FGL J0034.3-0534PSR J0034-0534?uÁŠ8tKû?tµU‹ò%é?ïÔ|ëh?tµU‹ò%é?¢(c¾çR@?»ãD3V¹j?îÝyÄŠÛ?»ãD3V¹j?Á|*lc?­…됚ã
?ë õdþ'>?­…됚ã?8¬g"h‰A?3zOQ:Ï+?ïüês
rï?3zOQ:Ï+4FGL J0101.1-6422?ímU&—»–ÀJ]c
'SÀ9nŸÀ<]
þÆD@3q¾‰=?ýút?¬î ‡—Æ?ÙÁ9d@+ß /µÐ1?ýMÌôåŗ?ïçlá)Ñ
¿Ï5¤&»V¿Ûò ›ìZ1¿ç"ò5<!ï¿ì«IúõÕ¿ïþó%&*6PSRPSR3FGL J0101.0-6422PSR J0101-6422?|Ê}y.1?ˆ«ÅgÜ?ïÆxë
£?ˆ«ÅgÝ?ƒýpº¡1š?‡iõX~+?ï°
={:?‡iõX~+?'5z'$2?‰KTÁ`?ïnT.Æßv?‰KTÁ`>ðá¨lMº>ñÞVgÿ?ïÿÞ=¯'>ñÞVgÿ4FGL J0102.8+4839?æ"UâyÀ,VÏ d#–À8ê0IsçXÀ;Óg'Æ~@Ý«PÑ(Ò@:Ì}?¬¼FÓà?Ðàâ"@"Ëê¡ô²?þ
þÙy•?ïƒÂwß5¿ÑØ)ø!¿ÝãJ<º¿âàe0¿ëÈ°ÞY½¿ïÿ¶Ï4†PSRPSR3FGL J0102.8+4840PSR J0102+4839?j×s;©Ó7?ctFœŒ§?ïå(ŒÄV-?ctFœŒ¨?>q[hr?‡o"?ï»':'^?‡o"?Žï?(`	½?†xñT?ï"C^Ù?†xñY?DÈJF?9"Á{q?ïúÿ
íx­?9"Á{q4FGL J0106.4+4855?ïdöwìÀ+½í6´ÈÀ8©Œœ[úÀ;áiF·G@h'"ß-?ü#iüóÜ?ª]é?IA?Ýg.!üT$@/&VÍl.ý?ó½ÿšT‰?ê]»Çí¿¿EQîµ)î¿Õ™ –ö¿àçÉÉã¿î"Yáó¥¿ïþ¥AÃnÕPSRPSR3FGL J0106.5+4855PSR J0106+4855?q<ç®T³?qºÍØ
v?ïÝç†0£W?qºÍØ
w?uùþd±˜?'á'áA?ïÔà6œ?'á'áA?‰nýïR?~I%ávA?ïšDB·ù?~I%áv8>É+Ì@Ÿ>'-¨"?ïÿÿˆÛPÏ>'-¨"4FGL J0205.7+6449?ÖCå0"(@¨Âa8ÿüÀ7n÷u³À;)®^L¼q@\íó@g™¼Õ?—Å
`¬?çQéßú@$wFˆz@ªIâøc¿­Èl뻥]¿à'5ÏŦ¿æ3ôÄb›¿èD¦ÃMÈ
¿ë~gä맃¿â²Áô+¶gPSRPSR3FGL J0205.5+6448PSR J0205+6449?éô‡àÍië?ÂT4ª<IÐ?È-à|ÊXW?ÂT4ª<IÐ?¬OÊêzÖ?ÆædxÙ!?î;QX^Ò?ÆædxÙ!?é¨ìåIqW?²è]K	«x?É\LjÚ:¥?²è]K	«y?wšLÙG¸À?gfêšà}…?ïÐËfMpŽ?gfêšà}†4FGL J0218.1+4232?ÒJ¼bKŽÀ1"~"ÐÝÀ7Â>Nh‡À;aHt
@¿égã5@ô¸ÙÐÁN?Ø›À˜ê{?Çjþс½@)ÆP¤]B@á+'¿Ñÿ']<9¿ß-˜T<¿ä9‹!0Ò0¿çW_ã?€¿í$¯ÂzäM¿ïÿŸ‡ð#êPSRPSR3FGL J0218.1+4233PSR J0218+4232?ǼÌî€.?ÃÁó~ð"?êÌÄ_ô`?ÃÁó~ð"?'ŸkÊæX?—OàíÏ0¸?﷑'PÔf?—OàíÏ0¸?ß ')#Ä¢?¼…Cœg?à/¾ën¯?¼…Cœh? ½|4m­?NÓ‹aß?ïþô(<¹.?NÓ‹aß4FGL J0248.4+6021?ÏáÕ[,A?æ­Ü|m8èÀ8>°C)JÀ;
ïunA&@Íx¤¥Â@c]$žDú?°¯8½5Õû?áUÛ¿-ý¿@"ž9'û@¤»üoý"¿Ú\DNŽƒ¿Ú_
Q'™Ë¿â°£¡ZX;¿êuŒ\š5¿ð?ðPSRPSR3FGL J0248.5+6022PSR J0248+6021?‡N83
ÜË?²žNíé}%?ï¢Ç3Ȏ?²žNíé}%?…öü܊R?¥¥T¦‡?ï«Ì$×?¥¥T¦‡?¹ptãu–Q?¬m2y=$?ìÑñc'M6?¬m2y=%?!å£^§6¨?K¼'GU?ïþá¥ÊŒ?K¼'GU4FGL J0248.6+4230?í«ÏŒCÀ.£^·E|À;nµÀ@ÍÀ=%(H¦@S9›W3î@‹o"Ný?̓ÞC¢|?薈¢ÑPÀ@ˆšˆ¬âL?õ7xŠ*eÚ¿ïÿþR€ÖT?ïÿÿ>¹ú¿Ù¨ ½Ð/®¿áó¢Ÿ&ÌH¿ïÿwy´!¿î(zÝì¯ÁPSRPSR3FGL J0248.5+4232PSR J0248+4230?ÒLþƒ>ÿë?ÌÀþIހ?æـ¾`€
?ÌÀþIހ?·çaƒ6h¤?Ä8_DžMê?íϙ2ë?Ä8_DžMê?È(eÌc?®pëñdÙ#?éõæœç<?®pëñdÙ ?y"é´cI4?fqV4ûj«?ïÌØ,—9n?fqV4ûj«4FGL J0251.0+2605¿ïôÊ /|À=~‹;26À:!["Ì´À<{¸;EPl@ÝgX(àõ?þ³°fd¸ç?×ɵÁ?äãkªs±@9à0Và@fw@(d"?íº@£^>z¿×÷½j.G¿Òn2b¨Á«¿æÜ>¯¾¿îú!~ÕÈõ¿ïû
ÝԇPSRPSR3FGL J0251.1+2603PSR J0251+26?]@@v藍?Wƒ[;ç€Ð?ïñ_ßĈ/?Wƒ[;ç€Ð?'¹é"}:é?˜+Áiôλ?ïr0³\)?˜+Áiôλ?–v¢ø¿8?ˆNAkëçd?ïLJïˆ:?ˆNAkëçg?v9œ5Yv•?cw3'Ò©?ïӌǕM?cw3'Ò©4FGL J0307.8+7443?ï3´G§Z@,p&grÕàÀ8Ûö"o³íÀ<Gö-fÿ@aßÀšdp@ã!ž¶9?§ãÐÊ][Ñ?ã¾]~
qô@1õÜy@àTÍâ?Ò®íÞë2i?Õgá:Âõ¿Ö"ÛÅc!¿æ_f¿ï¯âjmÝ¿ïÿÞ§À£ÊPSRPSR3FGL J0308.0+7442PSR J0307+7443?Iƒ@-¬š?Dš¼'ç?ïù¾Ÿ/ô•?Dš¼'ç?cüFüŒ?~¨Aï:ò…?ïì¹oõ?~¨Aï:ò…?Œžå(»¨?}pZ¡£?kŸ]?}pZ¡¤>u¶°†H?>z‰Á,/-Ù?ïÿÿԒŸá>z‰Á,/-Ú4FGL J0312.1-0921¿ï®:6©Å¤ÀJ/]$žDúÀ9ù…¤ðñÀ<ýdDM@JXE;st?ýίá»v?¾¿<ÁQnˆ?ãª)Ÿ5ºÍ@!»/fÊ@>Ï5ݲx¿ïÿÿÊPË?ïÿÿÊPË¿×,åÜhKC¿æÊ{ÿÒs¿ï*Aò闿ïÿö$´ë/PSRpsr3FGL J0312.1-0921PSR J0312-09?Ÿ
Êt`.?±]Æh$߀?ï¯9¬\ÿ?±]Æh$߀?'ÈÂJ!Í"? Ç¹©ÜD?ïq¹í®ñ˜? Ç¹©ÜD?µÔx?¶aü?¤·ÁÆa¬?íEpø	3Á?¤·ÁÆa«?n[VH)-˜?`ȐÍt*õ?ïᤩ·ÖÑ?`ȐÍt*õ4FGL J0318.2+0254¿éÂD6'²†ÀEË]9–ûÀ9ËɪiÀ<yÿ–M´¿@Ÿh#ÕÈ@lŸÞW8Ì?·Ô=À'o?â">¾°@ ã§Ú¤ý@–ÝàE{¿åC%ÿ˜üç¿Ç×±j¿×Ïxäl-¿äË»À5Ö¿ïÿúÁҝǿïÿÿ" 5•PSRPSR3FGL J0318.1+0252PSR J0318+0253?•Ô01Çpø?»—Ù[ôdi?ïQ^~qÄx?»—Ù[ôdi?"àù!9?°p2îAM?ï`ÿð3ö?°p2îAM?š·£Ç_"?K>)W™?ï/¢BáÅ?K>)W™?€ý)Dœ‰?m†	Û[h?ï¼[Ší?m†	Û[h4FGL J0340.3+4130¿ï¢`–@XÀ&%kÊSvÀ8ªµr£ŒÀ;ö5©/8Ó@šV=#vþ?ûVAU4æ?§ÿ	µáMã?Û¨Ÿ{°Ðm@/ŽŽ}Ü¥?øŠi
/®Ä?ï¶úÀoÇ?–ôu=å¿Ì?€Êë¡¿àÔÀŒ!·¿ëÙ-ފf¿ðPSRPSR3FGL J0340.3+4130PSR J0340+4130?‡™ÜÒAu?«fÔ é
¯?Œ¶û¡?«fÔ é
®?q©GjLzð?{m7!²´´?ïÜ­q+g
?{m7!²´´?Kô>û°?ŽIK";$?ï} _þ#?ŽIK";(> t³^)*†>£'à–eUø?ïÿþø´Ê>£'à–eUø4FGL J0357.8+3204?êYÿ>çÛÀ0{ÃŽÀ7qJEžpÀ;…¸èz0@Oð}+#ð?ÿÜЅ¾ñB?š"éß,Jâ?â{+ðHÒØ@B~ÉÀ¨Ò@ÉD"'Ô0?¢Žmìl¥E¿Ê¾Iý$-‡¿ã#³In¿ìXœ¿úÙ¿ï»x¡§Z"¿ïÔ+Á#÷+PSRPSR3FGL J0357.9+3206PSR J0357+3205?vhϚ%­Á?v~Íj˜e?ïÓ.`Ë´¥?v~Íj˜e?dg¨*
X?xSêzÃÄ?ïë˜WÕõ?xSêzÃÅ?µHH"w?§ág•G\ø?íVöýq?§ág•G\ù=0Xí#=F!pd/?ïÿÿÿÿÿ(=F!ŽK"r4FGL J0359.4+5414¿êǍÅ#=?ìR«~H…UÀ8¢xíÀ;€k©œF@۔œê@öß$¾%j?¯!ÇÐ䉂?Ý»Ÿíp±@'"M‹¤
'?ø…ê ²?Ö×Yƒ)Ì?äêÞÐÛOG¿àá@!X?¿æx'vµi¿ïDJ¢Ž-¿ïÿü9¡â=PSRPSR3FGL J0359.5+5413PSR J0359+5414?4(ÈÑîgU?5)!#(ÆE?ïýzæåÂ3?5)!#(ÆE?VPShÏù?bÆä«A?ïôÿWÖK™?bÆä«A?'±4Úµ ?Y»mâ5â?ïµ;/¨•+?Y»mâ5â>´iPRjNÅ>¬n´y¦õ?ïÿýrÕõ±>¬n´y¦õ4FGL J0437.2-4715¿Þ¡C؛Û>ÀDû† ˜'\À8Ǽ_—?LÀ<F…½CÃ@¿bå¨eå@lBHyì?¨žÕ˜£O{?à™ä½¯M‹@1ђً÷ð@Cå²÷º?ÂÉ·Ùö€û¿Ô$¼øÄL¿ãþ´;Œ¿í^•a¦Ž¿ïÿØ'sâP¿ïó?B5.¶PSRPSR3FGL J0437.2-4713PSR J0437-4715?Š^F˜d?ˆR|ÞÍ?ó¾åŸ?ˆR|ÞÍ?ƒ(5)dts?‡gUš"Ó?ï³_+Zn-?‡gUš"Ó?ÀÚÄrÓ˓?²"ÐÂ_?ëÉNãK
?²"ÐÂ_>šzF—Úw%>¢&b^¹i?ïÿÿ,-ËB>¢&b^¹h4FGL J0506.1+5028?åj­Ì ŸÉ@îcŠ	À:ÚD«*»•À<ÝR‹¾@ œKZÇ?þá='AŽ@?ÏÍseÓC‰?ïmß«÷@H±il«@"0ðÇ(?â
—Íç¿à¥Ã=×Ñä¿ÔÄAéã?µ¤Va
±à¿ìmc`!¨Ç¿ïÿ°_ïÉPSRpsrPSR J0506+50?±T!•ô `?³L`ÊÑ?íÕ{ÍA{ó?³L`ÊÑ?'ég¥ÑÕ3?°×n•
?ïh´ÂÑqU?°×n•
?Ô R±ˆáÐ?²ã'×+ÙÀ?å¯Ö§;?²ã'×+ÙÀ??]-1Åì?'SÕ|€?ï~–qÒ?'SÕ|€4FGL J0514.6-4408¿Ð?ÔRæªÀA´^=¢ø¾À9ôËbi¤À<EÌòŒyö@Õ÷É$̓@X2%ìù"?¹R"¡?èԜ9‡
K@#W>«6z?ûÝr~øƒŠ?ïëý^åé~¿Ï͍çߢ½¿æhþ0Q׿ð?ð¿ïÿð ¼x—PSRPSR3FGL J0514.6-4406PSR J0514-4407?ãÙJÊ_	?ÒÊà
¡62?ØMjkAíÑ?ÒÊà
¡62?ÇðÄ@í?Õóÿ'³?êÎÿoúÄ?Õóÿ'³?áN"´H¼?·oŽÂ??Ýbؗõn‰?·oŽÂ??À°"ø'Ï?Îacxñ?ëÓúZÁی?Îacxò4FGL J0533.8+6800?îû#	FN@2/À~à°¯À9j1ZëÞáÀ<`qªm@YZô˜B×?ý¢"#æ?²q¬?¹~f?×áäù~@#ûb(E@ÒÿZh¬<?ï½(êÚÔÍ¿ÓßZÃðÛ¿Õ³Üȃ<¿àŸÔçM"¿ì4 ñ|¯¿ïþ SPSRPSR3FGL J0534.0+6759PSR J0533+6759?|!uXoè?xâ|ËDI?ïÇã½O!?xâ|ËDI?tEÔi׎"?~5'¡¡?ï×tW,Pâ?~5'¡¡?öÕ]37?ƒ57BÜ£?ïPIUg?ƒ57BÜ«?[Teè…?Qq¬1?ïòUÍ7ý?Qq¬14FGL J0534.5+2200¿æhfêòJ(À ž³´ÎÀ4^ZXTÀ8u~¤˜Ñ@q?%3@¬À½ÊÑ?'
æÒ(ú?Êʖý'<@@ñ«!Z@GP÷iY¿É§•ßbÒ¿ÝÁíz—¿ãÑÖ!	e¿åÛ£>Þâú¿êô~ø-£§¿ïÿÛ¸"ÝPSRPSR3FGL J0534.5+2201PSR J0534+2200?ɱú°ïP?͙ßù­z?铁SÄ+ú?͙ßù­z?[ÿmÓå
u?zhJFÖyó?ïòI
z?zhJFÖyó?×coçOÜ?½-YÿI3O?äNH@X?½-YÿI3N=_¹œ¨'2=}Ó—´4?ïÿÿÿÿð$=}ÓJ í4FGL J0540.3-6920¿ïÃëó¢ûÀ?€¦—®ÞÀ8Pè¬&dÀ;1u§L	Ä@¸Ttvt@õV#"Cø?¥²žù)ø?ÔÆöôév@ ⟜èÙ@µ¬;ç%?îu×Ra̤¿änìF嗟¿ç	#•0~M¿çñbXdÆ¿ì6§â1¹¿î¤ZÝò%PSRPSRPSR J0540-6919?ÌìþRP?Ŝ9¹É;Ž?èù"ûÀkm?Ŝ9¹É;Ž?"k¥1§ ?"OÿWst?ï[¢ÖrÂ?"OÿWst?àÝÔ¬"Ão?´Õ>pv2®?ÞDV¦Öy!?´Õ>pv2®?u,6ÐeJ?`ßMµ}Ï?ïÕ§ï'_6?`ßMµ}Ï4FGL J0554.1+3107¿ïÿ¹Ûòçç@±@ìFÀ8²¥xÊìùÀ;êʉüm¤@Áj‹@êPÖ²(Ý?­áÀ,ˆþ?â+`kz¢^@+ýxÄ6ü?û£Z'"ÂÀ?ƒ¢=×üÖ«¿À.²šò_.¿ÝôÌÆÐ&¿éÞÿQš¿ïÿþBe«+?È^9Tš6PSRPSR3FGL J0554.1+3104PSR J0554+3107?H¸¨¤?Rþú"–Ӑ?ïùÑÕÜÛ?Rþú"–ӏ?`Jn³gö?‹ÎÀ§gÒ?ïﵑLá—?‹ÎÀ§gÒ?Ÿ$© $^?"eSRO³?ïÚ¶þßã?"eSRO³>¯bȌÆê>­yÁ—;S±?ïÿþ	Ów6>­yÁ—;S°4FGL J0605.1+3757¿Ä˜!óþ@ 
ˆ~¿#À9ÃÕ>ì¥À<'	µól@5&ƒwnL@ÖEüc"?»×²?>Ÿ?è¬kbNª@#ú<B¦m½@ý©¾Õ¾8¿ê§¼r¶?ï쎞"Ô^¿ÑU+@ªÀ¿æthAÝÅî¿ï{û#!m8?·!¶‰PSRPSR3FGL J0605.0+3756PSR J0605+3757?@'o°ÊH?@
Iٕ?ïûÛdߎ?@
Iٕ?r\¹ƒ."þ?'²Åÿ«›?ïÛFŒù¢Ö?'²Åÿ«œ?'¿Fõ¸Žg?€ñ'5óf'?ïrÈR;Œ?€ñ'5óf™?&ŽZ^ûì?·]G"¯¬?ïþ—šZ?·]G"¯¬4FGL J0610.2-2100?š#Æ(§0À2.8ÅCÀ9¶òÔô¹À<cÅü-ã@LÏõv9B?ÿÍø`ÏM±?¶žÕ)g­?àB««êÔö@"%p£×
=?æ'rhÓ(1?ïû®Þ¿×UÌeHÚ¿Ý+'€Íoà¿æš._8õ•¿ïÿèM[Óe?è:Î*šÞPSRPSR3FGL J0610.2-2059PSR J0610-2100?´í}¤Ý?Ì|wÊõ©—?íbPK}"_?Ì|wÊõ©–?"'5–2#?"/ˆaÎÀ+?ï¯c)§"7?"/ˆaÎÀ*? C—9†¤Î?•†YIYô+?îûƌg•³?•†YIYô-?
Lßþù?[݀É+ä?ïÿ—•™?[݀É+ä4FGL J0613.7-0201¿ïïA'RÀ"œ-IfËÀ7ÿ6)‡¸ÇÀ;…ë¾íç@¢fè¾Æ@#¹…È+}? Ñê¡|šŽ?ҁÝ$Þ±§@/Qߗª¬?÷ÚöE¿Â1êžCøR¿Ôœ¼C'¦á¿áTaì""9¿å8@Ž:–¿ï
žT}‹¿ïþ{›Ñ&PSRPSR3FGL J0613.8-0201PSR J0613-0200?jÐ
r"Æê?dÕae±D›?ïå/òÝ:?dÕae±D›?r<ň³F±?}âøÞ?ïۆtî™t?}âøÞ?zë:>i?…H"Ձm¢?ïŠSþ?…H"Ձm˜>˜ß(w+vÔ>œ"ü'¾«ß?ïÿÿ9¼F>œ"ü'¾«ß4FGL J0614.1-3329¿Ånû¢®°ÜÀ5Óä öñÀ6åʅʯ¼À;7Äe>Š@æ]êÁÕM?ùkâqy¿ß?Ç+?ÉÅ?ÒÅq"tI@Db0<î?û‡"»c¿ø¸°W™¿§¶™bDÌ@¿ÕoiÚº M¿àz4CÔk'¿êD_½Õ¹¿î>¾L‰"PSRPSR3FGL J0614.1-3329PSR J0614-3329?pBŠüO¤¯?ef1>Ðc?ïßzê`µ?ef1>Ðc?gmèիӂ?€á,í^%›?ïè'*T.?€á,í^%›?µ° ²Ðp?«^	¹w Ê?íIûé¥þò?«^	¹w É<Ó¸ãŽ8ãŽ=<O©<?ïÿÿÿÿÿõ==
*ëÞ4FGL J0621.2+2512?̼÷Ááb@L–F(~À:õ۹ϚÀ<'¡Îò@û@ˆuZ 	 @mYO&®À?ÇéKó?ïÿÂWþė@ öHÇ@±B%¿â1؊p0ë?ìœÏCŸ'?¸¸Û¾­$f¿ÝèŠBŽšã¿ïìü‡7¿éL"b¥¼"PSRPSR3FGL J0621.0+2514PSR J0621+2514?Gh—WŽVá?K¸ùq™Pî?ïú%Ú*j?K¸ùq™Pî?u?2Û?l¾—…9?ïՁšIÅú?l¾—…9?¤ŽJ¸È<è?˜÷V=>A?î·Ts|0?˜÷V=>B?2¾§[Uµ?»ß8—?ïý¨+•J?»ß8—4FGL J0622.2+3749?ïôSJâ"@%òµÖ\À8ÍIï7ZàÀ:¯ç¯§"@ìáÖõÈ@E!Whœ¢?±qta{Æ?êQ\1Y@1p æ)•%@þ¢vb?ÛÛPޔËT¿Ð*~CQäN¿ã¤©,´"ñ¿î€úfc¿ïÿîÝÃÀ	?ïrbS—WPSRPSR3FGL J0622.2+3747PSR J0622+3749?±Û‡$Uq¸?ÂÅ*7Ä%}?íďuQÈ?ÂÅ*7Ä%|?}|©€P\¢?¤ɼò`ú?ïŬÿ_F?¤ɼò`ú?³¿ ê5s?£(œ€Ð…?íˆëâ¹S?£(œ€Ð…>kÏíß`sa>yv<t}~,?ïÿÿä0 >yv<t}~,4FGL J0631.5+1036?´:o?Ý`IôÀ83¦AGÈìÀ;qc´~ë@[áþ@и,+Ø?©%œq».?Ø 1ί%@+"ê»Ë?üg¿	ў?³½ŸˆF
%¿Çdëýi¢±¿ÙdÛ·K[H¿á~®üØ-S¿î œ˜Q›¿ïû¨¸Ž!PSRPSR3FGL J0631.5+1036PSR J0631+1036?m[ÏÕjrý?2"&(>?ïâ¤0*•?2"&(>?S$©Á` ?`—œºïù?ïömÿ«P?`—œºïù?R¥œA?…Û™gE´?ï}oŠ×?…Û™gE¹>²LËÕ
«>°¯Oì¨tå?ïÿý¶f…]>°¯Oì¨tæ4FGL J0631.8+0645¿ìcù.&s¿óêwTË3À8æpÆ;¹À;©´oÞµ-@Ây5v'@XºÍÆÈ?µúaŸF°?â.,Þ°O@"±P¹U÷ƒ?öT÷™Õ¿éâ—½#â?x6ŒGæ7¿ÎÁ ܙs"¿Þœ\W뉿í´bþQÿý¿å֔APSRPSRPSR J0631+0646?KZªƒw3Ž?G§©öY¿4?ïù)U_"4?G§©öY¿4?jKèÍÀØ?sZ¦½(×ø?ïå´ä2>?sZ¦½(×ø?~'ÄiB?"~™·l‡+?ï|Ç!ܶ?"~™·l‡+?[ 4EÌ>ð¡K|£á{?ïÿ¿–"->ð¡K|£á{4FGL J0633.7+0632¿ä)sKdý¿íµÕڒˆ-À7\Wï«À:¾çW'Ž
@W7•BœÞ@Oú Âî'?–{Ûî}̊?Øp;7äs@:@¿ã°>?þ;Ÿ]¨Ò?侏½wÅ3¿ÀfÌ}F§¯¿Üv" ‹Â¿å½ýûC¿íï@?5J¿ïÿäA2¥DPSRPSR3FGL J0633.7+0632PSR J0633+0632?DN@ã÷ƒ?:漢P¢?ïúìoÏ?:漢P¢?J^RQNQ?]]Í>ì?ïù{hkk¬?]]Í>ì?ò€2ò;?VÆ"V=[?ï¸5ÿ47?VÆ"V=u=žWQ
yC^=²
<TÏ¥?ïÿÿÿÿ
G=²
<TÓÐ4FGL J0633.9+1746?íüý….˜Î@‰I`œÀ3G9"†À9)`ì©áæ@ÄTÉ@gëC°Xù?hC˜ÚLª7?×&v î@l8²êò@µMÏÁžÆ?Àaäáìn©¿Ã2äá¿ÚD+]ÑÂU¿äØÍ÷o7Æ¿î>FVüf¿ïe<ã.PSRPSR3FGL J0633.9+1746PSR J0633+1746?`îèì^³?aVLâҒ?ïï¡æ?aVLâғ?Fóèɀ_8?sML	¼IU?ïúC͟è?sML	¼IT?ˆq*(Ñ?~>ô«%Ž8?ïž;‡¯W]?~>ô«%Ž(?ð4FGL J0646.4-5455?ë3N½qxÀ6˜>·Ë³ÈÀ:º™I—#À<å³Ët9@áÞ¸1µ/?ý¤Uêî ?ÇïÂǺê?íuÉ næ@›ò9?ýJk±ò?ïøö‹â÷±?É|)WIh¿€|Àò+µ¿å…ؼÅÍ¿ïü¶ŸcÝö¿ïÞ?állPSRpsr3FGL J0646.4-5452PSR J0646-54?©^©žÞ ?³%%sF:?îjfr?³%%sF:?"±ð•Ë ?—‹¸±h°_?ïg:p{Q¦?—‹¸±h°_?´Û\å?¤oúÕÄF?í~äž|Ôb?¤oúÕÄG?o¦Ö¤N8t?`8XNõ?ïàY)[±Ç?`8XNõ4FGL J0652.9+4707?íIñNLâ@3¡/À:íu¶e';À=ÊC…Î@¾~ÜÿÊÑ@¥ð¿ñ7?ÒI·¤F›Æ?ïÿ³ß•ý-@[Ha˜¡L@,a$Wοã?ǖ,'?·†M¡sÙ¿ÑÄÌběP¿íðqJ¿æ´|¿Y=?–·Íûå­ÞPSRPSRPSR J0653+4706?»k\(`'?ĖGÅØÔ?쒔zóü»?ĖGÅØÕ?±Ո[dä?ÃjË¡.;G?íÝÅNô"b?ÃjË¡.;H?Ò(®øˆÿ•?·E"^6 Ë?æ먃»€5?·E"^6 Ë?«§uÎɍy?˜§_ė<?îEˆ£g(?˜§_ė<4FGL J0659.7+1416?ïÿކ`!­@ ‰3ÁÎl	À8U×øyùÁÀ;¹SšÍv@ÝœRÜq@§-ä>ÙZ?§¾Ûrýœ?ߏã=Qš@)vB||R@}¿|ØÚ¿±A)¶2¿ä°Iÿ}y(¿ì~ð€±a¿ï4mÙw¿îøÛH'¿ï§­Ãó	wPSRPSR3FGL J0659.5+1414PSR J0659+1414?åÇrÞùY	?×zÇû¾¡T?ÔqB
Mì?×zÇû¾¡T?…¼ZæV?¯³«h?ï©¿Æ"g?¯³«h?â4õ±nø?±7Mº¿–?ۖƝ"?±7Mº¿•>æ©›gj>æ«÷#({j?ïÿéíVd˜>æ«÷#({j4FGL J0729.3-1445¿à«ò™Çuc?÷x¡Åg~À9Ä÷øËÀ;|rïá¤Ë@§>9Ìu@÷µ¼g?Ä1§—ß]?Á°å^"
?ùÖ‡å</@c‡8îß¿ï,ýäò³?ì-Óbh*¿ê°ü¢'‡®¿ã\áb0!¿è´y"P\9¿Ü~ÒÃܹ)PSRPSR3FGL J0729.7-1448PSR J0729-1448?ï
g
ˆ?H7½I>?ˆ½|æ<žW?H7½I=?ïÂyžèú?¤Ìú³¹ª/?~Ã0‹øz?¤Ìú³¹ª/?î/gâ¿6?£$öåš2Ê?­	ÞÔš?£$öåš2Ç?ïVâ²?"±P\U?œ#©¿p?"±P\T4FGL J0734.7-1559?íM:‹Ç*\@')óÀ7Ít9ÀÀ;:¯ åS@³ËÉít@pM•ö?¢ž©_¨ß?ÑÒD2^ø@,ëXK±?ø¨©—h'忳ú§ü^¿Ú+ÎÛ쐿ã·'hÐy¿çpGüó¿í+/#:G¿ïÿå"m/®PSRPSR3FGL J0734.7-1558PSR J0734-1559?l·°jX?hV³/ý?ïãóHOp"?hV³/ý?Z€¸wêË?qFå¸Ã3H?ïò¿£ôÄ
?qFå¸Ã3H?›˜…†J['?'"¿ŸFOÓ?ï#;ÓÍ­#?'"¿ŸFOÓ>­ŠÀ"]>®nž'Z˜u?ïÿþ'Sþ–>®nž'Z˜u4FGL J0741.0+6618?ànª͋@=ŸØ{V¸sÀ:{ÑEØÀ<›'BCJ@͜ùöPª@
U£ ƒ™?½Q°vÕÊ?ÕR%'@Ôà—"ì@3bt>kK¿çT¶:º¿Þ*ƒaHð4¿Û‹ç)oe¿ä'£+Ó¿ì–ÿ'èÒ¿ðPSRPSR3FGL J0740.8+6621PSR J0740+6620?ÒmJŸAáù?Çpjs''J?æÉZ°_?Çpjs''J?ê–èŠñê?ÐW"ž¬½?Ť]Ô8Wë?ÐW"ž¬¼?¾˜ˆšÃƒ?©oìØÏ?ì,î짏?©oìØÎ?æ¥Óœ‰.?°‹~E²ý¼?Ò´YØÆí¥?°‹~E²ý¼4FGL J0742.8-2822?Ó-­€¦ŠÀ‰p"XðÀ8êÃ×ZÅHÀ;¶–F(~@&(Ûì@è&ªŽ´c?±vÊâ'Û	?Ôýåÿ"àU@Ôñ€
|[?ýd"äÖ¯?êV?rÖÚ¿²khó¥T¿âTB)Æ"¿ç¡Y{•£¿íOx¾'²!¿ã#͚R&>PSRPSR3FGL J0742.7-2824PSR J0742-2822?9ô5ZNÁe?4¾ñÍ'?ïüÁyT¶&?4¾ñÍ&?'Rå §M?¡¨ÈïÃó?ïuoXÒúÇ?¡¨ÈïÃó?†pé7:}¹?qH"›'?ï¦<[#	?qH"›‹?OcÁíü¡2?8贝iÓ?ïø'"€Ù?8贝iÓ4FGL J0751.2+1808¿¶ÁAþä f@5‰Å!ÞÀ9]oˆN»À<mByø¢@éR&ht‰@;ÔÂe?³²- ]iN?ç@Íàžö@+€Ïž8e@‡ùw¥¨ñ?ïÿ½OG"?驜œ€¿Äüì$Uõ«¿áà«aG¿îÉ=+¹É¿ïÿÈ¢› ÛPSRPSR3FGL J0751.2+1806PSR J0751+1807?YHl>ò—?Y Â'CÖÒ?ïó[Éà†ð?Y Â'CÖÒ?m¼R6øD?wox¯Wê?ïâ~C­É?wox¯Wê?œM^K…WA?"d.¸Ü/‹?ï•
£ÕG?"d.¸Ü/‹>µl—=Z'>°v{F·¢È?ïÿýRm_>°v{F·¢È4FGL J0835.3-4510?î*ÑØ®ÐáÀMCš‰ƒ¢À2{Èxª5ÉÀ8AA [À@ä¥}'ÿ@_ø"»ì«?gÖƒX/Y?Ô@Àæ"t@j¦[[Õ?øG>¾×?Ÿ
fÞõ¿Ñ``'çα¿àQúž—/\¿å£~IÜî¿ìö
Ù–ó¿îϼ5¥Ô:PSRPSR3FGL J0835.3-4510PSR J0835-4510?;­pLiÐ?B?iÝ°§Š?ïüŠQÿvt?B?iÝ°§Š?F¡ðí-m?oÙª¹¹b?ïúWƒÄ´º?oÙª¹¹c?'ƒuŸXr?^µ|ғÑ?ïµò)'Ÿ³?^µ|ғ¼?ð4FGL J0843.3+6712¿ï¦'Í®"@AÍÀÀ:hf9ñÀ<žSËY/F@Q¨¿&?û{Ɋ"-Q?¿-ý¿3?Þë¢ÐÏç@ªÉlÅü@Æfªƒø¿ç~è¾Dô§¿ÀB)Æ"¿ÆšXz"D¿×B¹ãæﹿé*æ}Íá¿ïðJ¶·ªPSRpsr3FGL J0843.4+6713PSR J0843+67?›Tc¹s? «J E³¨?ï%\â4gž? «J E³¨?Æ`	3øã?ÌÁ¢Û¹(?êgý³úG?ÌÁ¢Û¹(?Ô§D—,9?µ™ÓÂÕ	c?å¬]´iã~?µ™ÓÂÕ	c?¼u¾'^­<?£8-D˜ì?ìqH;*Y?£8-D˜ì4FGL J0908.7-4911?ïâã.1a¿ï™–òö,À8‡oó­â&À:{ýÍpa@XŒ­@C\ƪsÜ?»Ì뀗.?à—-¾ªN@!iÓpô@ ôÆ/$?ïo5ýè΋¿ã6oÞ_Fb¿å–Ÿþ7©¿ìtáMK¿ëî‰J–ý¿ïþ}ÿŠ9TPSRPSR3FGL J0908.4-4916PSR J0908-4913?IN•lÚ[?¨¨vÂ×È?ï}µ‹T™-?¨¨vÂ×É?Š	ãËÂõ°?®9á—h{È?ï—ØpÐô)?®9á—h{Ç?±˜ÇÁá?¡ì³Ð8U?íÌÿGÃÞ?¡ì³Ð8T?%ÿ3Týb"?Pü¨ô*?ïþ Ê°)?Pü¨ô*4FGL J0931.2-1906?îŐ 2žo@78ÿûÎBÀ;Ñ‹èÀ=nda©h@@¸MŽÔ@ºÃ.¾Y?ΦKÄ#°ß?ïûK€1È@æ…ý¢ý?ø^ Ò]…l¿ì"Ì3?ïïWq\?¶Q'ľ5…¿çVü\'¿íü'Ÿ½J¿ïæ#뗓/PSRPSR3FGL J0930.9-1904PSR J0931-1902?ˆ<2ù(E? Cè2Ïüy?ïŸ4ƒ`? Cè2Ïüy?ŠD_¢ŒÚ)?œéÒµ‹?ï–îu̗?œéÒµŒ?¶ÔâýK¬?£ú…ÍÿÖ{?í=c V‰?£ú…ÍÿÖz?K»~Z°v?8ã=ÛÜ`š?ïù>`iT?8ã=ÛÜ`š4FGL J0941.1-5429?ރrhã$¿ô‹'!¬ùÀ8úH…ªÏLÀ;µÛSñ@Þ)–|Y@Kh¢×0?»–ûÁÖz?âüÖö@"§â?$Øý@«<UEצ¿ïí×Äw"?ïÝ̙¡&V¿×?›ÜÀ¿æ{:ˆ&*¿îgý?[_¢¿ïÿýFKêPSRPSRPSR J0940-5428?†HF!~½?''ToÔ)F?ï¦Þçz?''ToÔ)F?p{§øc0°?zWL¹·"?ïß°9Ÿ?zWL¹·"?¥¾™ ek2?œ¼½—4³?î¤eù©L?œ¼½—4µ?FY¥h"ý]?6cd)ô:Ó?ïúi–¥Û?6cd)ô:Ó4FGL J0952.1-0607?È¥!Ôª°"@A±tÿ†]}À:È5šì€À<ÇÃqÚ7ï@xJ7[·@#3vO¶?ÇqØõÏûU?åÑneZÎ@›"ªNô@¼½{¿í½FG.?ï«᛿Î">ï)¿åû«©g¿ïÿþÐñ?ïÚ?›Ü?PSRPSRPSR J0952-0607?¿[—YŽ-?ÁŠ>Eø?ìÎ:[?ÁŠ>Eø?Â`ñ"•pK?É2öl`©[?ëgÛ£î?É2öl`©[?µUãÀ²3¡?£¬wÒw¥?íUC‡é¹Œ?£¬wÒw¢?ȕ£uÖ?³˜éß!£T?éڗ=â¿K?³˜éß!£T4FGL J0955.4-6151?â@Y1›‹Àø*ùÀ9ª¨ââ¸ÇÀ;ñ롤*@ŠÍ²¥Ú@ ` SÇþ?ºCSyO?ÔÐ=ºË˜o@»­ˆ["@ۄl5Þ3?ïZ° F\¿Ñ,b´€%¿á/âjmÝ¿æ:"ÀÅ¿íÎôÅ9Z•¿Û‹<¿N	"PSRPSR3FGL J0955.6-6148PSR J0955-6150?v9ÕVߺ?uÇS]­&?ïӌUR@‹?uÇS]­%?´ÕM6°)"?ºO³\p÷?íeVY)úÎ?ºO³\p÷?'ìÒàßñ¡?††eÌþŸà?ïh™hùs?††eÌþŸÖ?ÁUMýeò?¢K¨SµƒÐ?몟¬€¦"?¢K¨SµƒÐ4FGL J1012.1-4235¿ä;OЉ@&u֝0'À:ˆ­¹OÀ<u¦N³Â:@,mÇ-Ñ@PwFˆz?¸c±€@,@?Ói^¾Q^í@»hH¾µ³@¬OТÅ<¿Öc[ïêß¿áöуòÖ¿ák#>ô\‰¿áSµõòð¿î¹ý‡»¢¿ïþ÷÷óÂPSRPSR3FGL J1012.0-4235PSR J1012-4235?­­ØJÚ«k?­r†8'á?î%"{RUJ?­r†8'á?Â̑-X÷?ÊÕí$²?ëL۟´©Ã?ÊÕí$³?Ãðc9²ø?­Z"]kK7?ëç1"\ƒ?­Z"]kK8?Ôcû0<uå?®ÈF6 ?åÎgáÅ
?®ÈF6¡4FGL J1016.3-5857?Í
'¹ötÿþõ™t°¬À7dÿŽÀøƒÀ:;ƒo‹©@>ôŒÚ@cäõ8?©)·ßTä´?Ô°ß¼ÀL@$ŸÖ¶Zš€@'ð,¯?âã-ÌÁå?ç.ãBZ¤¿á×ûnÕ÷¿ålÚß4-"¿ì3Ô
2îj¿ïÿÞÝpˆÿPSRPSR3FGL J1016.3-5858PSR J1016-5857?@ýþªþfo?Dˆ:"á§D?ïûÀ€U@g?Dˆ:"á§C?bús-ë?pÔ·ÉëU!?ïíŒÒðï?pÔ·ÉëU!?…¤`ëc?z‹íöQTó?ï©mÂ|SŽ?z‹íöQTú>ó7x« üQ>ë4Wþ¥y?ïÿّ¨¾>ë4Wþ¥x4FGL J1019.8-5749?ݽÔÎt&¿åþ-BƒéÀ8u2_Μ±À:'
´©@ÿ¦|V@¬øCsW?¹Ü<ŒAí?Òhm
&Ú@Ýø?A^o?ú[çW´³?ï…/‡­¿è³ÿ ‡	¿ãíê‰v5ç¿ãØÇ«â¿ì:"å$²g¿ëDõÓVTPSRPSR3FGL J1020.0-5749PSR J1019-5749? €h§,v©?»ª©Fà}Ò?î÷ùu8–?»ª©Fà}Ó?•q)6ž'·?žn^¥‡A?ïTv¶Kq?žn^¥‡B?µž­¥tÉV?±@4Ս%F?íL*KQf×?±@4Ս%G?^r@Ói(4?Jîõ.¯?ïðÆߖKm?Jîõ.¯4FGL J1023.0-5745?®Ÿºf¿Ùv0¾ŽÆ'À6¦|µ]DÀ97Ó«ä@•#/Úä@W†Üþs8?¢äý› Ø=?ÖÐ6
Ù—@3hî9.÷?ön¼ÆÅKÏ¿Ì,û¡ ¡‹¿Ø …Üxfn¿ÕMý¹Ô¢"¿èq_=Ó¿íÇHɝmd¿æýsþÕ]•PSRPSR3FGL J1023.1-5745PSR J1023-5746?mÞI Ž?¬&¶ˆ¿?ïâã!¶ßr?¬&¶ˆ¿?LŸLþÝPú?]‡Ü­ñÄ?ïøØ,ÀH«?]‡Ü­ñÄ?"Ð6üø$š?oͬÅ_ú|?﬿$m?oͬÅ_ú~=ðÇfKX/ò=ù1²«O?ïÿÿÿÞq4=ù1²«¿4FGL J1024.5-0719?î.슫Uá@D?_JsÀ:&­czù›À<nÌ¢Ûa»@²r'å¢?þ6"çƒ1x?Á …¸Ò?ÛÛO\¿l@Ô»ó¡M@'´ªA2?ì<+)yv¿àš®×ï?¾¿ÖrÆ{ÏÚ¿ãfŽàV¿ð¿ÕÉg}ΊPSRPSR3FGL J1024.6-0718PSR J1024-0719?®Ñžû%'?´ô"´ÜÁŸ?îî¦M§?´ô"´ÜÁž?ª/h†^
?³wQQF…¬?î]	—š!?³wQQF…¬?¸ñX~¸"?§êՏýŠ?ìáÔüp(ï?§êՏýŠ?¿Ý±'
éî?§"HyÎp?ìIϾBÃ?§"HyÎp4FGL J1028.5-5819¿åö¼¹Ky¿ßz0ÓJjÀ6
\ËOÀ9ëQ=à5_@J.%'E•@%Uœê†ò?'Z,œ@=?ÑO>šõ@<g†ø­?ûð¢l¦òH?ë\âŽÕñ9¿×•Ù[%•'¿áåNšDº¿åu'¾´V¿ë«ä<U¿ï$à>ï~þPSRPSR3FGL J1028.4-5819PSR J1028-5819?=Æén›à?EPP p`ù?ïüG"Ò, ?EPP p`ù?H4í°(Q?Y#îñǼñ?ïùòēõû?Y#îñǼñ?"•þãíæ?cAiô>óì?ﯩ¨pH?cAiô>ô=eZËæÙ`=|½òª~ª?ïÿÿÿÿê§=|½ò«Ÿ4FGL J1035.4-6720?̘ü&AÀ`n¹ªÀ8µØGTRhÀ<µ™ª`'@Œ<‹v–4@ÿ‹eú/Ü?©Àc‡ä»?ázM£÷Á@0o¸dàT?ùL•Xí,?ïöÎ}üÛ?͔àwN–¿ÖZÆ?iøA¿æžvx,¿îjÃê¥ü¿ïÿüoQÇsPSRPSR3FGL J1035.7-6720PSR J1035-6720?Uéƒ=Ǫ?T<s6ô?ïõx>a?T<s6ô?r®Û€l?€ÕùK
ª÷?ïÛú¢Hÿ'?€ÕùK
ªø?"¼z¢-У?g×^Æq.?ï­wH½?g×^ÆqM>^sô*gV>`Yí{êÍ£?ïÿÿðÆé>`Yí{êÍ£4FGL J1036.5-8318¿ì JFXÍÀ5'"»äG=À:Dã)/¤2À<‰æ¤å'7@óú0ÞP?þÿ ÜïYÀ?½ršÀúËR?àЍK­}|@Ž½'¬î
?ãq÷ÝØÊ¿î7ûþé?ïýÖZHŒ¿Àí ÂWÓÑ¿æ6™ºPÉF¿ìDŽ#ρ¿ïÿ®¡hšôPSRPSR3FGL J1036.0-8317PSR J1036-8317?Ìwܖ˜?ØÆÀNRU#?èâ;»ÚZ?ØÆÀNRU#?"#¢ÉéÝ?¥ùÇH«?ïfâ±?¥ùÇH¬?¥_¢I3Ša?šÁU8_?îªÛlÇY?šÁU8_?>e8ÃnìÅ?.¼º|ÑcÙ?ïü3Xç'#?.¼º|ÑcØ4FGL J1044.4-5737¿èÇzt1ßÍ?ò€]£IEÄÀ6õ€ø¸ãâÀ:jýKð™[@Ôä'±@ΕY˜øŠ?œËux–Ùe?Ôb«Ü<Vr@4B†ƒ<`@J€y·üÜ¿¼3@®ñÅ¿Ûv·¢CC¿ã9Â~•1U¿ç
ŸÎ¿îYD_*‡é¿ïû•"d~PSRPSR3FGL J1044.5-5737PSR J1044-5737?Q ë<ê?I>"éʇo?ï÷ož*až?I>"éʇp?KÎÒ]fÿF?\Dú©¶Ú?ïùKh¦A?\Dú©¶Û?¿Ÿg¤?…ÔÔÞdá´?ï‰͂ap?…ÔÔÞdáÀ>Aá²AHâ>J–;œG3?ïÿÿû‡"p>J–;œG34FGL J1048.2-5832¿š=p…"'?â^$ãåFÀ6_c-תÀ:?aÀxi@ýÊE³é@Ñ$šéû²?'[r¹ÓBT?Ò¦‰l$ìI@<"™(Z'@"›NÐrŸ?ï:$n:¿ÍõX‡*¬&¿â5¹ö0s¿åh2^L¥¿ìºr•;f¿î¥¿—°
PSRPSR3FGL J1048.2-5832PSR J1048-5832?DëâB._?g8"»bx?ïúÅ{¯u?g8"»bx?E›÷t÷[†?VkûÇðÑH?ïú™"Â)?VkûÇðÑH?'"=ÊyŽ?Y-=ãÞ\\?ï·wÖÈ?Y-=ãÞ\=uZ[Œ·n=•f<Ôےo?ïÿÿÿÿÕL=•f<ÔçϽ4FGL J1048.6+2340?ì5E½uhÇ@O0¾
í)À:5¸H±JÀ<X•âTô@®°¬Õá@5^³¾?·ïðh]a…?É^KòK@
yT!ÀD(@ª¢€s?ãÛÀÛ|é¿ß‡¢u‹G¿ãwr'dÈ׿âðc	º"å¿ïÿBu?ïƯ²	ÒèPSRPSR3FGL J1048.6+2338PSR J1048+2339?â3O'³2?Î5"%/á?ۙaÉ°™œ?Î5"%/á?êM¸¼÷U,?ÐØ5L*(A?ÆÉ"«P?ÐØ5L*(A?à5fD?¾Õã>?ߕ3wæßá?¾Õã>?é¦û"hnÙ?³öÒïŠþ?Éd²^D›?³öÒïŠþ4FGL J1055.7-6028?ïʖY¯Ð/¿çŽ2BrkWÀ8¬À¾¡'À;˜À¤ @SÃvŒÏ@*]Œú?·³%ë!!?ÔÀÎý(µ+@x_»Qz@êǧŽ?èþ2Ö!ª¿ãÒò䏿ÕØǁß=¾¿åÁßԍí¿ì•ªåò8¿äaSlŽž"PSRPSR3FGL J1055.8-6025PSR J1055-6028?f(ëäï?l"è´öFU?ïé×îm?l"è´öFV?í£O¸&?›NáJ•™+?ïˆIrÃõ?›NáJ•™+?ž®+Ïß@?"iÚ(P{æ?ï
Ž§Ñ?"iÚ(P{é?lÎ w£*,?\°T'ú$?ïã1߈\Õ?\°T'ú$4FGL J1056.9-5852?ís–œ$q?èîš|îhÀ9×AšÕÀ;Å<¤ËüÃ@?bØè9@ìåÜhKC?Áü	ÂÌn?ïÿæÀ
@"vsBí»?ö–£Þ S¿ïú˜i²?ïþW‰SÑ8¿Ò
è@EÀT¿ì2j€§ZL¿ïÿû-2h2¿ïÿ'¢."'PSRPSR3FGL J1056.7-5853PSR J1057-5851?")iC2Y?µŠ@FŸ¾?ï^´µæm9?µŠ@FŸ½?g7¡ÌQ?uÒÿàÅti?ïèÈ^3äþ?uÒÿàÅti?°áʹCó£?¡õÖ,¶n­?íãƨׁ‹?¡õÖ,¶n¬>Åzz^ÜÃÞ>¸Q¢RþNT?ïÿú¡ahJ>¸Q¢RþNT4FGL J1057.9-5227¿ïÕwY*@•ÜÆ?À5òtBÇüÀ:ÄëQóÛ@¿àqoXþ?ÿé}£~?†NY²×`Ø?áRqQ{ó–@TM)Ür\>@'Îunl?˪OŸO'
¿¸/g¡¤Õã¿Üà"È×˿钂¹ƒCí¿ï¤ƒ!Ýö@¿ïÿª9ú͑PSRPSR3FGL J1057.9-5227PSR J1057-5226?^·™?Ï¡D?XUt3aɚ?ïð¤3`/?XUt3aɚ?:Kô)'?Uä.ß¡?ïü¶ºÎ?Uä.ß¡?ÄºZ®??‡2á³OÀ°?ï€í•Gñ?‡2á³OÀ°?ð4FGL J1102.4+0246?ïü"$$¸÷@K+J#9ÀìÀ;NVCÙs¤À=Y/F>©@b«@a¼þl'?Ô¬Ù<qËI?ïÿüÉï£@5‡†qž©@'H¿·e‡¿ìäšHì¿ÚØÐ;AI¡¿ÌoDö³¿ìoç¨m¿ïÿþˆ0»Š¿äðŽ¾^:PSRpsrPSR J1102+02?ïHc%Øa@?¦ýé@ÃÓg?–ó›DóØ?¦ýé@ÃÓg?â[ƒµ ?Öõ‰K¥?ÛHø•¾ÅÄ?Öõ‰K¥?↻[T\?½ÅПèr4?Úò‰IáWI?½ÅПèr3?ÎâPBºøØ?´o=÷y-	?èGkïQAÊ?´o=÷y-	4FGL J1104.9-6037?Ö³5¶²kÕ¿ÚQ¡GãÄ`À8HzÿzŸÀ:Æ:¸b²@áTzU±@õ´'S+÷?²×f®µµ"?ܼñBM@"ëQX¸'ú?øß',꙼?êÃ'ëk¿Ó?¦n£¿ßÌ! Œœ¿å‹¡¿ï¿íBÞô¾¿ïÿÿ)@k*PSRPSR3FGL J1104.9-6036PSR J1105-6037?:(€äêE?7Ò¸®H?ïüºïãb¼?7Ò¸®H?d'Y"™z?pˆ~?®nè?ïëØo¦lf?pˆ~?®nè?'ϧÈ_¼¬?f¿=•è3?ï´Á`ށ
?f¿=•è@>å
%X'Ò•>یïáؑ?ïÿêõÚ§~>یïáؑ4FGL J1105.4-6108?¸ï••ó[j¿ë˜<8dÀ8°8\gßãÀ:â¤itš@È(MQ@eº|h0k?»ÈÉ2
™F?Ôō]¡í@Y:´0ô•?ûÓÒ¥~Õ?ëtž½ÅÈͿӌÎû%OÆ¿ãê™fmó#¿çÔoŽ-TÍ¿ë€<01öó¿ïÿþ½à ¿PSRPSR3FGL J1105.2-6113PSR J1105-6107?u{ß\Ÿê? Ì•ˆ
?ïÕÑAFÁ? Ì•ˆ
?…£±"K?£ž^³I?ï©q9ûvÓ?£ž^³I?‰üã;""+?~âYÖßܤ?ï˜s­³?~âYÖßÜ­?;¤'52?*T͓ød>?ïüž‹o¹`?*T͓ød>4FGL J1111.8-6039¿Ú©=u'¿¼$(ÿ'½ßÀ7—V¸sytÀ:'o™ëÎñ@ <|k‹iU@ËŲý?§hìÁ?Õgùä]K@*ß¼@ùý‡?åEfîVŠ¿ØÌï,¿Ø>("®zý¿ßw»B¶³Ü¿éêœ÷+°¿í'T·PSRPSR3FGL J1111.9-6038PSR J1111-6039?BžEÃ~ë?9oþÄõöû?ïûXn \?9oþÄõöû?R˜nø°?`s"ÉC©¼?ïö³Èöp?`s"ÉC©¼?®9JÑ}C?£L¡¢£	D?îkRè+Ð?£L¡¢£	D>ÃF˜HCüÅ>¿ùáà™$?ïÿû.Yíî>¿ùáà™$4FGL J1112.1-6108¿ãw.á疿á8­€¬7×À8•nÛí÷À:g µí7@ DØÒ³'@¨^=¢ø¾?ƪ^û'?Ͳ 8¯žê@RÎ-±ê?ñk	Ãù¨¿ê `þG™?ïKÄúpt¿çcÅ×惿ãíNL"-I¿ìTA ´@¿àÀ*ݤ5PSRPSR2FGL J1112.5-6105PSR J1112-6103?•ßr·+dƒ?´Îã$$E?ïQjF¤Ü?´Îã$$E?ÞDÙ}'?¡DYÈ+?ïy
Ù4x?¡DYÈ+?·ŒÐ"øuã?¥bñä-?íeï`ñC?¥bñä/?H0Œ??áþ\ß@?ïùóû>½þ??áþ\ß@4FGL J1119.1-6127¿ïúû܍#"¿áv"Ž¾À7܉ð¯*%À:ÀY‰QÞ@iœÄò7ë@J<d4]?¨ZàÜò?Å­7Ü_ï@;ÕýÍö˜@È¡Îï?âèˆ6ê?Ôkf€g™l¿ânE1by¿äärp_äl¿éBpˆ(X¿âÕð'3¡mPSRPSR3FGL J1119.1-6127PSR J1119-6127?·²
R·ˆ?»>GK±t@?í	¾U¼i?»>GK±t??ÂŽ¼#…?ªke<æ´?ïyëŠä?ªke<æ´?â2r²™ß?¶¿O\µ?ۛšÌüC?¶¿O\µ?…÷ˆÔ?ö?r˜ì©—Ő?ï¨#µÜ¯?r˜ì©—Ő4FGL J1124.0-3653?Ês	‡Bù½@6ÁÁBá&À9#ˆ©[®À<JDÇ°-@óG;¨Í"?þOU!š"?¯Õ?Pç"?ÕÄ C@%dBAÃï®@¿é³¸SÄ?ïÿQŸ/пÊ
Þdú«'¿Ú¸©>Ó$€¿á'Þl	¿íR«ž~Ü¿ïûªÐù'7PSRPSR3FGL J1123.9-3653PSR J1124-3653?|îÄYg&Ú?yóƒ(žM?ïÆ"wM1²?yóƒ(žM?r"¢ÆÛÛª?|ž8Êvü?ïÛººrHI?|ž8Êvû?•åېα6?Ž)¥§g?ïPÑ#yŠw?Ž)¥§d?,ú'TÕÉ?#—L³4Ó?ïþ0W×ê´?#—L³4Ó4FGL J1124.7-5915¿ï¾–8'Ñ8?ü;V¸sytÀ7"^±f>ùÀ;ÔoX}p@!õÅ¿g_@_Á}ä1?!§"Kâà?ÎêõVÙ«'@(y!S6ß@-¨ìô-¿Ç®†»›w¿Üf9e&u`¿ä0&8xí¿èöÚQðœ¿ìÄw…¿ä®ÑnòüâPSRPSR3FGL J1124.5-5915PSR J1124-5916?jâ6I"<?i¶Òª(ó?ïåɶël?i¶Òª(ó?`T8'«ž?wFA\̒?ïï«ÇmTb?wFA\̒?¦ãJ1ÞÅD?C¼(e¬?î'Ë\âª?C¼(e«>äi°4Kf">߇fø?ïÿë–O˵>߇fø4FGL J1125.6-5825¿î°\Úo@À¥º9LRÀ9׋œ€ÕÀ<T›ñb®@ )c:âÔ÷@CüäŒØ?Àž":ê?᏾ˆfk@­'"ª?÷«]ƒé¯¿Ï"'ª>˜?ǗOýÄ;"¿Êµ_]]©)¿ÚHE¾ûþ¿¿íŒ*¢k¿ïÿ¬óéqHPSRPSR3FGL J1125.3-5824PSR J1125-5825?S±ô
OÍ?RÕÀ±™7?ïö'þú×?RÕÀ±™7?t4¦iÕî?€{}1^ƒë?ï×ù–³,T?€{}1^ƒë?ž*áӀÕþ?šp}œYyÂ?ï¨ñcùR?šp}œYyÁ?R4
ÜDš'?;´|îZÙÅ?ïöåú'ݳ?;´|îZÙÅ4FGL J1126.4-6011¿í­Ñ\Ë1$?îÅ2@QÀ:"ä;~[PÀ<?‰öŽg6@j­b#`­@Êþ§°´?ÑGAˆ
¦?æ²uhaé)@¤X9|ùP?ü÷s¼»1Å¿ïÿcW¾,÷?ïý(IË%-¿âÖ斢nT¿ác¿ø¨óª¿ïÿÙi"A'¿Õ›Ä¡Û¡PSRPSR3FGL J1125.6-6012PSR J1125-6014?×é:¤z~O?Ë%IÑjj?äb­ÂÀØ?Ë%IÑjk? IPË<<É?¯#p£[k?îûjóL<3?¯#p£[k?܄ÿY~"?·ýn­3:?ὀS@ž½?·ýn­3:?¢+Vƒ½?µ?'K¡'XW¸?îÝJ—Ä,?'K¡'XW¸4FGL J1135.2-6055?°©Ë£ëø?Ⱃ`št‹À7Ð*o?RüÀ;4Ôóâ»@'±«^="@+¯EÓHè?¢XèàÞk?Ò<(…a9@&é䒼/Ç@>óp-?Ó3ÊnJ¶¿×M†00It¿áõÖ±R¿æà@è'œ&¿îiΛ&%¿ä±úƒ¿<ÁPSRPSR3FGL J1135.2-6054PSR J1135-6055?:@a·ô$?,®Ö€‹@¾?ïü¿÷óÉ?,®Ö€‹@¾?_Þ3wú¥?lV3mSÉI?ïðæ@D?lV3mSÉI?…ÕE,©?q¶Yœ²mÚ?變ªëO"?q¶Yœ²mÊ>ìÉ\Åç>ã	]—Â?ïÿã6îë£>ã	]—Â4FGL J1137.6+7527¿ï§²£¬0@DeìÃã?À<ÝLvÑÀ=ž™Ó{<·@ ,Õöí@dÀĀÍñ?Õ¨ß<ÿí?æ÷]ßÚ¾@
Dr¦É¢?øçý%	O¿ï–­94?ïÿ—Yοо­dҒŠ¿ßv•¾BÆN¿ïÿ¹‰#)Ñ?·%—"0ÏPSRPSR3FGL J1136.1+7523PSR J1137+7528?ìdþÛZ?Á…ˆTÓ?¼Ø!'%3?Á…ˆTÓ?ÕU"š°K?Ôµ½Yåß?åU=²§þÚ?Ôµ½Yåß?ãDÌáj]?·ö¿«E׶?Ùvf=Á+E?·ö¿«E׶?¬79j…?•%Â$Yƒ0?î<Œi_÷°?•%Â$Yƒ04FGL J1142.8+0120¿ì,t®f@Mµ\î À9Î{€©Þ‹À<F@îݘÍ@=5?§á?úñўå?¹Å‡Gw8?ՆhD7@P<«ù@ëpTü±—?ߟy'wéñ¿ÒcÀ"?h¿ÒTÑ]Ö¿ßÛAÖNV¿ëêòòÑCT¿è:"DÇPSRPSR3FGL J1142.9+0120PSR J1142+0119?…Ý¥3.ÙÝ?³ Áþ?降k3D™?³ Áý?¼úÀùe?ʐîÿÓe}?ì`¼àÝ3?ʐîÿÓe~?ŸE! Z	Š?™Ä•)<ƒ?ïÖòý/³?™Ä•)<€?®VŽ,N¥?–ٍ~²ÀŽ?î—>K?–ٍ~²À4FGL J1152.0-6107?ëÈ$W'Ÿ7?íwƒßóðþÀ95èºiúÀ;£ã³™ @XZÂnO@±æ­j1?¹œ÷rë:?سµÄÈqs@™eéŠs@HÑQkØ?èÎ{·?ïÚ&ò³c¿áªjÂkŸá¿çQ.ƼèS¿ï
¸Á?Èñ:j_kPSRPSR3FGL J1151.8-6108PSR J1151-6108?H}©l­Åó?A'¤u=a?ïùà•¤Ô?A'¤u=a?ž6µ¿+?¸ÀžA×y§?ïKòRÆ?¸ÀžA×y§?Ž,CèÿÎÌ?x´£Èº"@?ï‡Nð\Ä?x´£Èº"H?loœÅT%°?[ï+'ªÞÈ?ïãc:«Ú?[ï+'ªÞÈ4FGL J1207.4-5050?ë)Be@&՚•BÀ:Ô©: À<€`mþá@M˜f"³@ˆÌ»ÑÓ?¿Úø‰"ò?䂓=_ @E"¼»Ò@»ž`²?ë­2h2?ïÆÖÖ¿Õ^ü· =¿åÜá­¿îXO·Î8¿ïÿ™"{UPSRPSR3FGL J1207.2-5052PSR J1207-5050?9[ev».M?4Êâ4_"?ïüԓQ(š?4Êâ4_ƒ?Z?ÿŸ@?†qÃA	S?ïÁïK€À?†qÃA	S?''25æô?€ØRìè‰ö?ïsvnW¸É?€ØRìè‰þ?]Š3}G²‹?L¼~hUm?ïñ:æA\&?L¼~hUn4FGL J1208.2-6237¿ìž§ Ðkd¿Æ©¸J´¯À7ýùp™ÆÀ:'Ӂô@ùx}À?@'í»YÝÂ?°jýNõ±r?Сzäw¹J@ ™íZáÍæ?ÿÏ懳é¿íå`³I?îïV.྿ãäÅø¿ä9€ô¿ì[`®–€à¿ì•†z$PSRPSR3FGL J1208.4-6239PSR J1208-6238?I!n"ÿQ/?F¸îçíÍ?ïù·¤w@,?F¸îçíÎ?j<ßçÖ'?u$bø?ïåà )è?u$bø?Œ[DÊ£ ?<"µzX?ìÕsÌ?<"µzV?ÌPâQ®?r{®W2?ïÿIxíx?r{®W24FGL J1221.4-0634?èËF=åî@KÂFŸ¸À9Ûò¿¥œÝÀ<E¿çáü	@îFïÿ@‡ü¹#£?¹_ !·"?ÕîžÄ%ß8@0T9=@dø7^»ø¿Öǁ¿gR¿ÖÌP:ªö¹¿Þ²«£Ý?a¿å{ºÁ1Ž¿îPüD‰¿ÂVjoàb¬PSRPSR3FGL J1221.5-0632PSR J1221-0633?l®Œ?`ÑU­]?ïÁ'È£Éó?`ÑU­]?º!äê ?ÃøG•£a"?ì½ÛÃb¾?ÃøG•£a"?'gšÇá2'?'Çe·îç?ïtÃ)Àöl?'Çe·îå?Ê5'ªbøÌ?¯qধç?ér›•gAÌ?¯qধæ4FGL J1228.0-4853¿ë¶äª(½w@+Hˆ/À8ƒ—‰!SÀ;gFvš@ÛýlR@,M€¼S?¦|)`y	?ÉDã^߉@rT¶"¥@<Y¹YÓ[?ï®K75÷3¿æ4€ãÀ.¿âb·O
¿å¢•Ä¿êá,À¨QB¿ïÿ}ß(ïãPSRPSR3FGL J1227.9-4854PSR J1227-4853?뇉.ó¿R?¾m-¹€?ÁáÛD1·?¾m-¹€Ž?æõÔüމ?Ø@:«ùs?ÒWÎBî?Ø@:«ùs?å»Í~ª.S?µõtÛ0Ï?Ԉe«£[?µõtÛ0Ï?Ñ}:]¿óI?²³7óÙL?çAbÑ [?²³7óÙM4FGL J1231.1-1412?ï3¥-Íø±@H0!¼jÀ7[ñ˜^À;WÔGëQ@Ú¸æ;é?ù—¡øìx?"äùБ?Ûü}¿sré@G1ïÝëÙ@	÷ï†á>?Ô½C¢—7?š¤^ˆeXŽ¿ÔŒËÀ]RÁ¿ã†€¸!D¿íîˆwÆ¿ïÿÿ&¦³PSRPSR3FGL J1231.2-1411PSR J1231-1411?¸ ^
þ{D?·×$Å!ty?ìûô> 0™?·×$Å!ty?pœà¡ˆ€?Œ~"î"?ïÞÆ?ú¼ñ?Œ~"î#?¹KŠéó?©Ú­iE?ì֟î¢ÏÁ?©Ú­iD< žZ¹	á<Ñ÷÷Z'ö?ð<Ò™¯b}4FGL J1253.3-5816¿—&JAm¢[@Y˜*ŽÀ:0%™È"À<
9¶Úó@Z¾bѱc@C'ŸÐ€?Ó ¡ ¤%?鍺}¿ÉY@
}œãÐõ@ÀÁ­§n?ëˆGô·M¿·á(V¶E¿éü…%Ä¿êÍñŪ™œ¿ð?ïÿüÉï£PSRpsrPSR J1253-5820?ÐË{åd?Δ¹8b·?çðšBz
M?Δ¹8b·?Ó8ÔŒýš?Õ~í˜K½'?æc•ó92?Õ~í˜K½'?Ú÷w㏏½?·ˆe²«3Ê?â"D88"?·ˆe²«3Ê?´Ò<Pd'7?§ôØñtc?íe¸uóm¹?§ôØñtc4FGL J1301.6+0834¿ïd&|Õ+¥@Q҄ßÎ1QÀ9¨b/ ¼À<[å¯ò¡s@íJÛp~˜?þÚÙÕÉˑ?µ`J~ºW?ÚLó£¦7ã@ ÇTŸ"…^@^¨¯à?ÓÙp^·ÆU¿ÉÉ<Ê`¶Ï¿Ý"€ÐÊÞ¿å£ü~Á&&¿ï
ý˜F³¿ïÿ±[W>«PSRPSR3FGL J1301.6+0832PSR J1301+0833?…»œ{G?°© )b¥?ï«¥Žã?°© )b¥?§w™ÛuÒR?½®…€ÂÆ?bH¢Ú?½®…€ÂÆ?¡T@ƒZòP? ÞÎvñ?îê»÷ÊPÜ? ÞÎvï?y~×ýI$?hÇÃ+³,r?ïÍQÒm?hÇÃ+³,r4FGL J1302.4-3258¿äŸ… ®c#@=ØOãm"BÀ9>³"&jÎÀ</#qõâ@¬–"¨q?ú£2ü¬Ž?´ä!s€?áì(¢‹…°@(žZWdjä?ò–"VŽ­¿ÖZE›ÀS¿Ä½¯¸ê¬¿É€Äápó³¿à%°"±"L¿ít0Ôý¿ïþ/{ÎSPSRPSR3FGL J1302.3-3259PSR J1302-3258?cwû
"?b!ïaY??ïìˆûòß?b!ïaY??{¥â²)؅?2Œþ³£?ïÈ´:›¬N?2Œþ³£?ž<‹5[
U?šB+;c_Þ?ï¦U'–?šB+;c_Ü>Ú¦P}•œ>ÔÁbNRiY?ïÿò¬×Át>ÔÁbNRiY4FGL J1304.4+1203?ä¼TL‹J¡@R¨¬1'À;cجëÀ<ñI{t¥@?Ž7£@2[úҙ•?Ï}$"®?ïfAý{k@<o"͊b?üw­ñ•Y¿êÕ>¶I(¿à»J>³‡¿ÁW)‡Óh¿ëìÀ|ÝK¿ïÿ>ñØJ?àæ.¢=PSRpsr3FGL J1304.6+1200PSR J1304+12?±æhéÉC?¸•ð·õ?íÃ2âÆ׎?¸•ð·õ?±‹ÅÈ÷—:?Ãm½ñÊÉ8?í·Fá
?Ãm½ñÊÉ8?ÀG…E‰Bi?«Ìt)ù?ë¯f?«Ìt)÷?Ý?[pˆ8?v\lAð´?︋'=à?v\lAð´4FGL J1306.8-4035¿Ëi¨I@6-gý?[`À9wòŽþ5%À;ܱ?¨Œ|@­•£•ÆÑ@ìgßã*?µÉɍ'Ei?Ãð˜Ä\Ð@¯Ê]†ÃÔ@ZMxß?ï÷¡!MW¢¿á‰Óˆ¨°Ž¿ä{=ï홿ãX)Âq)8¿ïÿø]Ê5™?Ø®'úîôPSRpsr3FGL J1306.8-4031PSR J1306-4035?íÃ
i£×x?µ²«©Þ{?±ç"²áD=?µ²«©Þ{?äô¹1h)?Ó,/¡$?×ڍ/«?Ó,/¡$?è|÷Bêv?°µºS\}?Î#ªôV'?°µºS\}?è*špäN'?²Ù7œ3G?ÏU–<nż?²Ù7œ3G4FGL J1311.7-3430?ïoËg‹‰¶@<,Š›ÏÔ¿À7…H-–;@À;fDH.lû@̓j5©@X²éÌ·Ô?˜¨yÜ9ý'?É!@ûBV@0 À~á@Ü4ÌesÍ¿›÷ý8`ªÌ¿ÚºìDâ2:¿âp·ù1¿ä²tË•¿ìËLd\ ë¿ëˆG◺FPSRPSR3FGL J1311.8-3430PSR J1311-3430?¤,™Ï/3õ?¬fÍC"õq?î½6c
À?¬fÍC"õs?mÄÛÝ%Þ?wìÊçä/ž?ïâ;$"÷Û?wìÊçä/ž?Ëy'âÅ&Ý?·õxT¼
?é!¶N¶I?·õxT¼
>¾E°™œO=>ÂJNó¢šc?ïÿü7IìÌ>ÂJNó¢šc4FGL J1312.7+0050?éž‹¾@Oœ1&éxÕÀ8ö6êÀ;øždÚu,@Öþ~ö€$@ŒÏkã}é?®>—?w9G?ßBÚ$ú
s@,mXê|àü@́±ñTA?æêZ±ý=®¿Ã)Ê(ؑQ¿ÚæÝR¿æAP—ÈB¿î釃 U¿ïû	h^ŽPSRPSR3FGL J1312.7+0051PSR J1312+0051?pd‹<þ¡?¨R´Æ'Š?ïß6é‡À?¨R´Æ'ŠŽ?ñ9Oq?›,É,Þý?ïˆ;ÎÂ;?›,É,Þü?—ž4MPÊ?œ{ü/†?ïCž]•z?œ{ü/†>Æ Þ£­ð>Æøè°0m?ïÿúwÈW<>Æøè°0n4FGL J1335.0-5656?á?ÜØ6É@­µR\Ä&À9œVwÛÙ°À;ÞIWaç@``LpñÛ?þÊﲪâ—?¿ç¾€-â¼?ÚÓíNL"@^aIÆóo?ù;¬Îª?Ä|*ˆiÆm¿ãUeÂÒx¿ÖT¾\‡¿à£v'id¿í¼<e›:¿ïÿ¶Ï4†PSRpsr3FGL J1335.1-5655PSR J1335-5656?}zN]A?uvyŸ3ƒ%?ïÅÿÿcD?uvyŸ3ƒ$?¯)ÛJô?¤û4	ÆpD?ï‰CX"¾Õ?¤û4	ÆpD? àÕÕuTå?"õ}Ñߛ?îñò¢¨ª±?"õ}Ñߛ
?•GW'½ÕW?€öüBd?ïUÅCêU?€öüBe4FGL J1341.7-6216?ä¯Þ€À=Ð?—F~ŽŠÀ8><ÓG:À:$ƒÁÁ@y'w¾'˜@»ÒÄ]''?¿®áÕGšž?½ðÍÝîÞ@'Dé>?ÿŒü?O?ïl™Pž~¿à¼ÃÕ­F¿æsY>	Ðä¿æ0šö奿蛪ëÑtÒ¿ãä"ŸR¹PSRPSRPSR J1341-6220?ÐכÒ)PÊ?Й·Š¹¬h?ç"2ëW›?Й·Š¹¬h?ÔPÒ>>ãŒ?ÔT—ñ¿oø?åזààŽ;?ÔT—ñ¿oø?Þ³^¼J37?ÁFºÿwº?à¦P¡Úæd?ÁFºÿwº?ċIlú"?®ÄçEÒĀ?êÝ:-¤Áw?®ÄçEÒĀ4FGL J1350.6-6224¿ÒI½Tqœ¿ÔæÒâÀ7ÞÓMŽFÀ:™c²VÿÁ@[Ë ýQ@EE\*£B?±$Dÿa?ÚyJn¹?@%sçÑ5Z?ýoçáüú?îlT‡@с¿ÑÕ­+ª~¿Ý,iÀc¿ãÛJ^H	Ú¿íã}zV¿ïÿw¿1cPSRPSR3FGL J1350.4-6224PSR J1350-6225?/4YRj} ?#ÏðTÁ±j?ïþºjÙY?#ÏðTÁ±k?Y+ó,ú"Ü?ch1Ut¸{?ïóji'¶?ch1Ut¸{?ûɖ+l?W'½v¡¯?ï¸ñÙ§R?W'½v¡¯¯>Ð_`Û]Ïg>Å; Ž|"ï?ïÿ÷ÐO'R>Å; Ž|"î4FGL J1356.9-6432¿Ûÿƒ£\©Àvò"º7À88É$¡ À:ÿ§Ÿì™ò@eÌ[7ß@?ÛÒú
x?±Ar'?Ö,?Ž‹Hž@çE™›@m¬¯Ëà?Ò àdõ"¿Ù¿v"2á¿ç>	…º¿"¿í*†Pçy ¿ìϦ›àœ¿ßŒ"2T;PSRPSR3FGL J1356.6-6428PSR J1357-6429?eiå?qT?d¹Ð2[8_?ïê–ðÀŽ?d¹Ð2[8_?‰'ðW¥ž?'LÜâQ¦Ô? >¡j?'LÜâQ¦Ô?¶YÄP,e'?©N.5vd?í4ÇuúsZ?©N.5vd?Jè¬\,äG?7µ˜e}ß¡?ïùEÔèôÇ?7µ˜e}ß¡4FGL J1400.6-1432?îôÚ`wãØ@FˆÚãæÄÆÀ9ɽaõ¾^À<Jã´oÞµ@"{±|9?þèm!kŠ"?»R´¾õ.ý?ÛRËêN½Ó@üC}-RI@zßæ¯÷Õ?¸µÓ9£¿¥TºÂ^3è¿ÙJT¢nªX¿çŠ×^÷\¿ïÿôa¼2¡¿áÎ"7blÝPSRPSR3FGL J1400.5-1437PSR J1400-1431?}/̂c"?€c/HvUD?ïÅ¡ðfû9?€c/HvUD?š±¶íLd?¢yCIû?ï*rH—œ?¢yCIû?›NWøì?Ž±=2ä4?ï%G¸8œ?Ž±=2ä5?–ÕÂúB)G?†oõ
ÆQS?ïIQè-îµ?†oõ
ÆQS4FGL J1402.7+1306¿ÅŒÖ,ŠFá@Q
Ž`€sXÀ;/´yï°'À=Ag2>@­@Ù0«ï\š@¸/ÿ¢/?Ïn"3¤?ïÿÓT¦J'@j†!퐒@¬ô•=¿¿ïÿÿ>¹ú?ïÿú÷''ý?wäò"䣿çVØ߬޿ïÿüÚ±'Þ?ïÿh@S§PSRpsr3FGL J1403.1+1304PSR J1402+13?ä¡*${'?Òiâïí&õ?ֽū·ý?Òiâïí&õ?Ó¾QÓ/4L?×Ã=âEóp?æ ×heÙ?×Ã=âEóp?ؗ±vÕå?·FìsR~?ã´x'D•?·FìsR}?²Þt3ÿ?¢è…ô͑~?í¾d1y€?¢è…ô͑~4FGL J1411.5-6133¿Ð­™‰ø6¿Ãƒ'ÓÀ8Žìø¼>àÀ:ZD4"@êýsޟ@1µ"±«?ʔk¿ù?×¥l`¦]ø@"Åyò4e?ô³[,°ã?é­Mî\ê¿ëPƒÀê@{¿å˜fÙS¿ç…NSJ)ð¿ïÿÑ;ÇVk¿åwÜ{~PSRPSR3FGL J1409.7-6132PSR J1410-6132?ç9Ñb%v?جá$O¡€?эÀ];µ?جá$O¡€?²HY¿•µ?ÁwG›xÜ?í¶ôÝè
J?ÁwG›xÜ?χ‡?²"Þ˜—@?è8^;:@?²"Þ˜—@?EMċÏj?7Kñ-¡€?ïú¬¸ÎÝ
?7Kñ-¡€4FGL J1413.5-6205¿ÊÍÝÏ5"ù¿çx;»²À6hz™#RÀ:lÞO¬@tðo"7…@ªWÂ^´Á?—ZâàƐ?Ö:[4GZ@9cœ¥½"K?õø‹Âku?ïêF$§5¿Ä:òÚ¨'–¿ÞK9º5ñ¿ã|¯ŒwG¿ëқ
7 (¿îÑ݉¦PSRPSR3FGL J1413.4-6205PSR J1413-6205?nÁöpoA?¬È<¡?ïá>	ø?¬È<¡?I¿°WQ{?X¶"ژ?ïù?"ê+?X¶"ژ?'?þ]&Cl?Xüüxcš
?ï·‹fò?XüüxcšK=|0–/Ébý='™­‡¯Ü—?ïÿÿÿÿǝ='™­ˆµž4FGL J1417.6-4403?ŽWcãÁC@0!æW¸MºÀ9~VG4À;õÐÕp	}@õèä°nG@wCõ"V?·Â<Pg?ÐÒpû•¸@%/ ×{|?üy/ï[íç?ìÃãNïQ\¿ÛÉ#…–,¿áíp¡'Øa¿â"Ànš'¿îà@$Ï¿ïýØ]y­ÁPSRpsr3FGL J1417.5-4402PSR J1417-4402?€+ëFlO?y÷7€™"?ï¿PRæNÄ?y÷7€™"?'Ê\Os9k?¤ ãí$Œ?ïi­"f3?¤ ãí$‹?œILýä?´¿0z}?ﵘßr?´¿0z{?§>ďóÔ¢?âØZS?µ?âØZS4FGL J1418.7-6057?å¢#ë ?À½ªÛ`cmÀ5÷'7ËHhÀ8¾èyÑ@ 
'e¾—@Ât֐›?uHऽ\?Ö]þÛß@6åÖZHŒ?÷¥óýhK?ÒJ»¿à€£ßÓ¿ÒRHù꽿åB
 À>õ¿í]+TB¿ïÿý`éNäPSRPSR3FGL J1418.6-6058PSR J1418-6058?ËÎÊvP´'?ÙÞSÜKt$?éMbkÒ÷?ÙÞSÜKt%?E†ÍT?WÃtSÔM?ïúž[Ì¿*?WÃtSÔM?"›'ºŸ^™?ŠeôÚ
'×?ïc#r+
?ŠeôÚ
'×='F¯(kÊ=¢«L‰"ñä?ïÿÿÿÿuÏ=¢«L‰›14FGL J1420.0-6048?éÜםŽÞ?͈y¡+´9À6­ûmÊÀ8·#24/²@ )Ve'V@üÉï£?³:à?Šj?Ô
›p3o@'^Ÿð˯–@`C¢?Ý?ï©¡ue¿æýôµÖ¿áSS.{=Ž¿æú˜'Bdÿ¿ìC[ªÌ¿ïÿöùŠpPSRPSR3FGL J1420.0-6048PSR J1420-6048?¹¿Äòiî?ÑãM™à8?ìÈa²Â=?ÑãM™à8?c•¶õŒQ€?"ÎŒ©ãS´?ïìjI
s­?"ÎŒ©ãS´?«I7ÜÊK?£lü§<2ú?îKl'3_?£lü§<2ù>ՐIˆÕÈ>Õ<ž'đ?ïÿõ7Û{º>Õ<ž'đ4FGL J1422.5-6137?éÜùÞ1Ku¿äº'J9À7¡77¤²À;
Pø@@ €iڏ-/@Þý'¬?¦¤§tù|?áØì`@2£ôDàÚ¡@l
%É?ë´‹g\?ïӍæÝð¿ÉdxÞ°¿ÚS'Yáæ¿ë‹%nú¿ïÿCý…Ò<PSRPSR3FGL J1422.4-6137PSR J1422-6138?2išˆ•=?-õ¯ˆ}?ïý²Ì¯Îî?-õ¯ˆ}?KñH»ZÌ.?[C*à6?ïù­Ñ)L?[C*à7?›÷]‰"S?•[ÇøF·™?ï Gųß?•[ÇøF·">"êc͒þY>,;ÓµÌÇã?ïÿÿþÑYÁ>,;ÓµÌÇö4FGL J1429.9-5911?Üä%¸Ð=?ôÜfŒ
ÀÀ6äh8éÀ:'u>p~@£3K[ô@Þ~pHg?˜Öoý'»ö?Ò¦¸¦¥@2PwxÝap@hš6Íq?ÎÐ
YË"¿ØÞ$þÜ¿äOC¿ç£ˆXÿ¿í½ªOÊB¯¿ì¯ÑêBÿYPSRPSR3FGL J1429.8-5910PSR J1429-5911?Bó/ƒtNQ?DÌY´rt5?ïûC4"í?DÌY´rt5?I‰TE›?Z[w'±Àœ?ïù¸*î»?Z[w'±À?…UˆÑà?kõú_æ€?ï©Ê©Ü»Ä?kõú_æ'>Bý
—Ö>JæÊ  'Ä?ïÿÿû_€¿>JæÊ  'Ä4FGL J1431.4-4711?íbS×rê/@(§¥	9d¦À9È9¼º0À;ã¥{O+·@x1ü@òR}{Uâ?Àª}—…m=?Ê®ÿ…Ö@%¼Cè@³æ¥;
¿ÙãEó¿Ý)´.pV¿éI-``gõ¿çH~ôÒ¥T¿êˆOúꊿÁë;¢ÃcíPSRPSRPSR J1431-4715?响øŸ$þ?Éûv"Ù-?ÔØäÁ¶?Éûv"Ù-?î}ûÕèáÐ?¶Öã	˛Œ?¨ B¡qã?¶Öã	˛Œ?æˆ÷üÐ1?¼kfX½)?Óòî_ž?¼kfX½(?íUмañ?›ÖiÞÎ`?µQzTðr?›ÖiÞÎ`4FGL J1440.2-5505¿å¿ºy¤'@%4¢žûÙÀ9ì"ì"qÀ;b–ãܳË@´"gÑK@óìÌG?àåîqbBë?Üdrûö*@?,0	³@"K>—ÀQ?ïdG!ý€Ê¿çK;gµÿ¿êLL¿vM¿í¹Ò9?Ö¹õ͔ô¿ïÿþó…õPSRpsrPSR J1439-5501?îèRǜ'?¥†}õç?¡zӆ=v?¥†}õç?ï3ŠùèM?³œVµ&É?™Ž Âö_I?³œVµ&É?çåRaäò?³ÿdYÇ$?ÑÂ5[<6?³ÿdYÇ%?ï\é%³W?Œۍ¨?"bß;I•?Œۍ¨4FGL J1446.6-4701¿Þ%üñ¸@&×W÷7ÚbÀ9¶Ë¢*aÓÀ< #‹öC@úÚý8?ÿq'Ñ8?º'pÉÂ?ۏç¿€Ë@L÷‡‹z@™·
ó³–?ï÷ €=¨¿ãœÀ€
V€¿Ú¢J"
¿å1&s1P¿íˆ}ˆkI¿ïæ¡à×PSRPSR3FGL J1446.6-4701PSR J1446-4701?lÚ~IxÄ?mšÙ¾€\.?ïã%¶‡ó?mšÙ¾€\.?"Â0Âóý?'ÔÚÆÊWW?ï¬÷=øô0?'ÔÚÆÊWW?¢-gëµb?–í&Òlîž?îÞ=)Dª?–í&Òlî›?ª'š3ä?u[³Ïê"?ïÊ«ë.`?u[³Ïê!4FGL J1459.5-6053¿ê­q™[…w¿üªØ>À6ÎÿÄpݹÀ:p™ÆC@›h,**@ՙÅ8ƒÕ?–ÝB÷݂ä?ÑsUAûÍì@3fÖE"@«"Ï€0g?ïÇ€\±²¿Ü ïCš3¿ä_Eà´á¿ç—×øyùÁ¿îVÁ"¸Ó¿ðPSRPSR3FGL J1459.4-6053PSR J1459-6053?…ّ²Š?±ÊmK=
à?ï«Ü™¹5Ö?±ÊmK=
à?a†Hƒ»E"?xÑÃùæÁ?ïîy·|D»?xÑÃùæÂ?¡ÉQԚ?š4DÚHr±?îïÎjâ¶?š4DÚHr°>!þ´&8ãŽ>."7Ãjæ?ïÿÿþà½>."7Ãjé4FGL J1509.4-5850?ì"Ó¤¿ã¶¡²lÏ6À6áÐË_ƒÀ:,…'¤Ø'@MÒ±=OA@$³"כ]?žœÁ}t† ?Ø¿Ì^<÷,@3¿â`²È?@¸l"}Ðæ?îrjJ÷u?ёÖ¤¿ÝìWڎ¿ä‰Øá®a¿íW®rn²e¿ïÿÑ ïcÑPSRPSR3FGL J1509.4-5850PSR J1509-5850?E.Œ¬®
;?Im'þŠÜ"?ïú´\ÔÔ|?Im'þŠÜ•?OÁÕ'Ìç+?a!êOI\?ïøŠ¶Æ?a!êOI[?‡'žÍà?%M›ç¤8?ï£`éÈ~?%M›ç¤+>6…6Ü>AÕY­jqÖ?ïÿÿý=ï_>AÕY­jq×4FGL J1513.4-2549?ìïuXÃ@:ö—Oß;À9±WVO˜À<DC;¾òï@ç笳@ÃÝ:ZM?¶ÿ‡_/es?۝}ÿµ,@³Ñà2_@6ˆ*?î˜?ËG¿É£u{S¿àBuüŸ|¿èÊXÿ°J¿êþÈs¡¸¿ïûý<aOPSRPSR3FGL J1513.4-2549PSR J1513-2550?KgU,ƒ'?BÞÕîÏkg?ïù8¦*´à?BÞÕîÏkf?'/qï¤Îå?"a@'àzy?ïv"p'Ù‡?"a@'àzy?"uډŠ¹?ŠÉJ	×b?ïdWI+³©?ŠÉJ	×h?y·*'ÛÊ?g	—Áu#'?ï̑«ÐúI?g	—Áu#'4FGL J1514.3-4946?·™·Aýu@<½±¦×À7ëýŽ5¸IÀ;t]ýâŽ@"ÜÅ×?ý;v­‡?¡UÑÿͼG?֖!_K?@1,M‡rO©?ûiùée‰È¿ßNa6ü–¿É‹¶ÂtYC¿Öå+ž{޿ߜjÄÄ낿ìë€K꺿ìÙä!þ£PSRPSR3FGL J1514.2-4947PSR J1514-4946?br©5¡™É?V\—˜¸4ƒ?ïíVÊ^g?V\—˜¸4ƒ?dÉN'Ý?F(À!Ä?ïë6±ùØè?F(À!Ä?‹þ՘ÚÁá?ƒ0¦õ+ß?œ"ù?ƒ0¦õ+â>'}St¬RÙ>ƒ®•Þ	)F?ïÿÿ¶
²->ƒ®•Þ	)F4FGL J1521.9-5735¿—Lµç"¿ÚZyMBÔÀ7N#'¬?À:ƒùd@ŸĈ/º@ûbó?£Ó›s
"¼?ÛzA—b@/I¯:ÎÄ?ú0«?ïҟà·ö¿Ñnñ$oöÞ¿â'†ø­%¿èç/N¢¿íázn['n¿ïûÓ {‹PSRPSR3FGL J1521.9-5736PSR J1522-5735?:Ñí׿W?4[¨?ïü¥ÂE	?4[¨?Q—Éhí®Ù?^Øh
0g?ï÷4K‰)?^Øh
0f?'ž6邳³?aë>ɒu?﵇$Yõ0?aë>ɒp>MAZFžæ>P¯Ty•yÆ?ïÿÿø¯©|>P¯Ty•yÆ4FGL J1528.4-5838¿ÃÓUÉü•o¿ü\¼™yÀ8Î.«6$À;›mµæz@ ¼Êv0^@(éÛÑLŽ?¸Ö—Péý_?äi›Ô×]@#»úëÄ?ÿ#á?¿të…tž?ïIšé$ò(¿Ômc°©€—¿äÀ|A™þC¿í蜁U€¿ïúÖàÌÞëPSRPSR3FGL J1528.3-5836PSR J1528-5838?lxI&yd?­âøœ¶—?ïㇶن~?­âøœ¶—?dº*Îî…Á?p´§ŸD?ïëEÕ1y?p´§ŸD?'º·¥­óJ?Z…œ"?ïµ!iH4?Z…œ">ö§‡rWŒù>å÷.…ö™c?ïÿÒ°ñQ>å÷.…ö™b4FGL J1531.5-5612¿îw…ïöϐ¿6pÇ¡À]ÁÀ8žo¿«À:‹Á#K^£@")K'ñŒ@E\{+‰?À܃ä{•"?âßøãú@×P +"@½(ûL¿ïûü€¿?ïÿþBe«+¿â@`xÜ¿éÚÔ,<ží¿í…H©¼ýL¿ïÿþBe«+PSRPSRPSR J1531-5610?€'ŽQÝ*?'Áœ9Â$†?ï¿aǒ¸Š?'Áœ9Â$†?~U«µ
˜v?Œ
"WXÝ?ïÃT¨•äÑ?Œ
"WXÞ?²(0æã?£åøØx]?íºùã#Ž ?£åøØx\?JX(µåòr?;‡Ìê?ïùiõ҆'?;‡Ìê4FGL J1536.4-4948?¸ÅN¯3á•@%‡CUÀ&À7D¾'wfiÀ;i
	Ó¾@4è-?þXAZ=c8?™t-EÕĐ?Ï¥}'þ®@48ð"aùð@+SÔhx?ïø$B`M¿ÎÒ&þÇp¿ÝÔÜeÇ¿ààÁKdW¿ê7Pþ¿ï-¨§b°PSRPSR3FGL J1536.3-4949PSR J1536-49?u–ô
å>ô?{–fÚÇÙÔ?ïÔÒê5ƒ?{–fÚÇÙÔ?wúvM?×?­÷w¡ep?ïÐÕe?­÷w¡eq?¶u4Ç©?¬?݇å?í1^¹g?¬?݇å>RÎ"Ñ">\ݓ(Ó¼?ïÿÿöúï>\ݓ(Ó¼4FGL J1543.6-5148?×5±¹<‡|@ù#zX‹²À8À/#ÙùÜÀ;3òuÓÂ@wP»¯C$@C‹«`k?¸ÓfC«Ñ?ÕY:Ë@7Tm?ž|@
jØf¿ãuIX8¦?ï³±=$M½¿ã˜Æ5¿åÃG
H¾¿ïP²4›@¿ïþ)ÉßPSRPSR3FGL J1542.9-5141PSR J1543-5149?QñߒÈ ?P6Ír€À?ï÷6±?P6Ír€À?†Öï¤
ª?¬°úéhîÓ?襤AoóÖ?¬°úéhîÔ?‰"û€ìÍO?~ñP{•"?ï›tüLÊ?~ñP{•?p[gÍy?`KTðivQ?ïßIá0e
?`KTðivQ4FGL J1544.0+4939¿é:6û¸¦@Izd×ñÀ:ii˜JAÀ<»´Ci@V3Á£xë@üÂ]Þ?¸Œk2ÓçÉ?ÉBÔ+'@ï|i+?ø
ˆ?ü?ë08AíH¿Ë|ÊÌ¿á"lhÞæ«¿ã_j^B«v¿èÈX>/'¿ïY§ÜR{ÎPSRPSR3FGL J1544.0+4938PSR J1544+4937?â,&}Í?É@}çÔÃ?Ûû˧³g?É@}çÔÃ?áë<
¼?ÔՑC˜É?Ü)Õû‡êˆ?ÔՑC˜É?çç˜Ð!&ø?²¹ža7?Ð0Î_½²?²¹ža7?ÕÖ´NÛ?µWà4BÚ$?垥Øô'?µWà4BÚ$4FGL J1553.1+5438¿æ§ËÉ®Q@G•ˆ†aÀ:—ù_ÒÎoÀ<Ìò8— C@¼<Vžó?ÿhfx?¾í‡¾‹ý‹?Òó†ŸìÄå@ïÒ¦*¡"?úݹv®³?ハŸ€¹N¿ÑMÓؿރ{Óö¿àïgAÒé¿îgÝÿú÷ƒ¿ïòO]‹KxPSRPSR3FGL J1553.1+5437PSR J1552+5437?¼¯üü÷Wo?¶¶¼‰é?ìj`a?¶¶¼‰ê?ÀRïhš?É à À¶ü?ëë{?D%Ú?É à À¶ý?¾çŜ™Ê"?¬W5lJ?ì#LlÆ®?¬W5lJ?ÃD"€1
á?¨þlîû‹?ë.Ûó¼‡?¨þlîû‹4FGL J1555.7-2908?݃®Ô³¶@2€‰ÁµA–À9°^©Ã)À<y)·‰o@¾€+ßVè@x¶Ë?ºˆá~<ò?Ï)U–µd@
\¶â¼y@X=®·8?Õ;Ä|FM¿Ý¢ˆá:˜¿é	ß|Ò¹¿é!YKË°m¿èÒUºc¿ïÿ¨âaßnPSRPSRPSR J1555-2908?Հ¹Œ}?ǪÍú%˸?å?£9Á9x?ǪÍú%Ë·?Խػøó_?ÏáÝY{Ÿ?å¡¢†P?ÏáÝY{Ÿ?à°vƒ) ?¶™*ο»?ޟÎù¬Â?¶™*ο»?ÝUè·`ˆê?²X3Š''À?áU¤O»‹?²X3Š''À4FGL J1600.9-3054?µZ0L[d"@0o‡z³$…À9¡çÒ␃À<lU\Rç.@!›_íP{?ÿd1m`U«?´£×àýz?ßü©ß7©@"ëØYÈÉ2@Ëuå	"Ž?ï´~÷¬Ê¿´FÕQ€¦.¿ÁÚâ9Eœ¿ÝUÈbÿ¿í]v¾"e¿æßnàˆktPSRPSR3FGL J1600.8-3053PSR J1600-3053?V,ˆ&6¤o?Pª¥M¿Éå?ïôé»ìä®?Pª¥M¿Éä?u®ç­ãJÅ?8c¸0?ïÔ¢0¤9k?8c¸0?–j2*( ?Èò[ÝXC?ïL®o^®¿?Èò[ÝXC?CÈ.ý¨YÇ?4–ÌÃ>—?ïû
ô@•é?4–ÌÃ>—4FGL J1614.1-5047?æf­œ£©?ǵ|N/7üÀ8ãpOô4À:2ðXõ@ ,3¦¹Ú@IèÄzô?ÊÁPlÕ?Ò(}ˆÁÛ@	²|¤–LÞ@:–ê<Ê6¿ï(å!,u?àכ³¿åWiþ÷Ak¿ä(àwúc¿ïÿðÇô ?ïýçAB?–PSRPSR0FGL J1615.6-5049PSR J1614-50480?×á—giR?ÔO8Íy=]?ä4wLKW?ÔO8Íy=]?Ã9˖
h?Ï¥Ë,ù?ë1|¥ü?Ï¥Ë,ù?Ñ·M«qÍ?³hp†+?ç$Y*Gu?³hp†+?Ío®¥"rß?ÁÅå'}@¯?è¤V›#H?ÁÅå'}@¯4FGL J1614.5-2230?æ䧜ë"@43Ä~I±ûÀ8fé†.ƒÀ;àş±á@ê×™"v?ý™'Í_š?©u}äI?ãMˆÿ˜|
@4f^‰"S?ûq…Þz?ï
–1ÿ?ëP6®è¶7¿Ä9h6¿ãªDâˆõ¿íCçì
õ¿ïÔ»¾²'ÊPSRPSR3FGL J1614.5-2231PSR J1614-2230?B=뎓?<C+´Î?ïûp¸E\?<C+´Î
?aŸ8'eÄ>?q8ïîôn?ïî`Ç}š=?q8ïîôn?ƒz¥v#(?chB×5?ﲝj'r?chB×5/>Œתd>§X¡Zî–?ïÿÿÿ…Ð>§X¡Zî˜4FGL J1615.3-5136?Õ¨üǒ=¿á>Ó°ÜáÀ8Ýñ¸> À:ˆ™|=h@@ *¿;>Åc@¢¡<ü	Ñ?µ°@¥½£?æDí¥Šh¤@&Xn\Ôí-@´€?ï gžÊ°é¿Ô†.B]•¿ÜÜ¥‡äep¿Þ$ò¾#Ñ¿í²
©§-׿ïþÊô<'PSRPSR2FGL J1615.2-5138PSR J1615-5137?,Ód»¹C¾?(&ÆhÏ×L?ïþ2É´Dl?(&ÆhÏ×L?Vكu¤'?aø
zó«Š?ïô">Ew®?aø
zó«‹?‹boëKŒd?ƒ"{vZs{?ï'v@RÑÏ?ƒ"{vZsƒ>Éuñ¥ÕU>ÁŠ$ÑÜ.?ïÿù¢¼C—>ÁŠ$ÑÜ.4FGL J1618.7-4633c¿ìÓ'" Vˆ@•ê˜+ÛÀ9=#I±À:©ï§Ã(@p{¥<åä@$º¼)?ÛwNëö]À?×» ¿þˆ1@±+ÿbKO?÷°à]"p?á'‡|a¿â8— B•§¿â[eŠ¿a¿ç™è^x±B¿êg‹"ôk¿×$*í"1PSRpsr2FGL J1619.0-4650PSR J1618-4623*?Ã2ïþª§?Ã]ŠÊóӒ?ë3DU{–?Ã]ŠÊóӒ?ÅŐ@4Þ°?͓î7$5?ꎛïòÈT?͓î7$5?ÔݤèY??·mIÄõ?å'-û‹Ó`?·mIÄõ?œÿYãý±?'¯ç"^`?ï0à#?'¯ç"^`4FGL J1620.7-4927?äP¶3æb§?ÙâûB+»À6ǎö¨hiÀ:hõ2F¤)@ K6r,@i9™m$? Í¤Ážy?áyß¿î˜@7©)þK?üÁ"À?ïK$£Mx¿Ù¨ââ¸Ç¿ÔÔg ÎN¿ÞØ<'g±¿ì>ß¿Ød¿ïº–ÔÃ;TPSRPSR3FGL J1620.8-4928PSR J1620-4927?1,630.?./µ¢Á?ïýÝúy9š?./µ¢Á?O­^Ÿµ‹?dP.¼Õԝ?ïø¨X½?dP.¼Õԝ?…ìîð?{õ[Àöñ?ï¨LD?ùÊ?{õ[Àöÿ=œ[Ü=ÃÜ>=ª]ɍáä?ïÿÿÿÿ!=ª]ɍá)
4FGL J1623.0-5004?èMÖ4H¿Ò©÷þ½áÀ7…J¼Ì¥À:†Œ"ÎX¾@ –üªàéº@Äہ›v?«öÍ&cìä?Ù±y_<{†@%¶å«ÀãŠ@;ùUkí¿ï'½ÂmÎ:?ï|µ«¬¿Ðÿ3ý2›3¿à«;³´M¿éú¿žæàt¿ì^|PSRPSR3FGL J1622.9-5004PSR J1623-5005?GÀÕ³y<õ?iš¹O|?ïúʓ!²?iš¹O}?YxƒóU'?e½6PŽáI?ïóvC¾U?e½6PŽáH?¦"(þB'‰?œ½"Ëß?îÝpÖè?œ½"Ëà>Ú6ÝJ¬×>ÔS띷/?ïÿòä¿Z>ÔS띷/4FGL J1623.0-0315¿Ò257<	@>«ÅXdE$À9'˜(€QÊÀ<&‹ÿ}#A@IèVk@3/‡­?³xýlÒ¼%?΅÷eҗ½@@,Meä`@±©'×	'?ïô"'òÜ+¿Ýa=@'¿à)Tݧæc¿â\ä¥5¯¿îvSCsó¿ïÿßÿY'íPSRPSR3FGL J1622.9-0312PSR J1622-0315?›úFwËø? Fä}=ö?ï -Ï,A ? Fä}=ö?¤´z?²@zWoî?î´¾Ø_?²@zWoî?½˦å"a?®@Œ| ýE?ì]¦‹#Os?®@Œ| ýF?°§`¦¥Ä'?'f³ ‰¯Á?íëë+Gn?'f³ ‰¯Á4FGL J1624.1-4042?Óð»ªy¼Å@©¡N™ÁÀ8P
ýÅÀ;fe€…@w?<ÖÊý@z¼¼´PÕ?©$'bq÷?Û¢‹EC0@)ؽ©CZÉ@8<­…v?ïúeA"_%¿Ñ,}a¡Ì¿à
¯	mg¿æ'"|ú&¢¿ï	OŸz"+¿ïî?CîKPSRPSR3FGL J1624.2-4041PSR J1624-4041?G÷÷"˜"F?K»KnÃó?ïúÙÚ?K»KnÃô?jôÇHí¸?‡Í›ÿc;'?ïåî8·?‡Í›ÿc;'?ˆ
Jk(çR?zÌZì[?ïŸÊÖS\d?zÌZì[>ØyÔRx>Ӗ)Ѽ?ïÿóþCï>Ӗ)Ѽ4FGL J1624.3-3952¿Ô@˜»nA÷@ÃÝ}8ÐÀ9ž3ÆàÀ;ž6`å@'úÇ[ô@üGÿsF?À¾Ëê'Q?Öàþ]ª¨@vì["@æßóÈd?ïý†ì]Œ¿¼vјŽ¸¿Þ5úÀñ¿áË8Bf¬Ý¿ïÿ›‹â ò?ïÞEedÞ§PSRpsr3FGL J1624.2-3957PSR J1624-39?°òuñ‡EB?±ú°0b ?íá±AÏX?±ú°0b ?¶¹æ`È?Æéŵ—s"?í(Ã>sý§?Æéŵ—s'?«ëK=P?œæ­šþÃ?îAKL/—?œæ­šþÃ?ų5V푠?±œ×Ìôý¸?ê"2ªD›—?±œ×Ìôý¸4FGL J1625.1-0020?ξ$ÞMžp@?Ö9.÷<À8žÎR
À<CN3iº@3ç}R;6?ý}›6QÌ?§™(c)"Â?áE"žæ_›@1â">iƒ?ýð´`Dc\?Ãa}Uì¿Ï§½^DÙÏ¿ÑÆmãv¿ãwlH'·¿ï¿¼¿ïùM^W¤,PSRPSR3FGL J1625.1-0021PSR J1625-0021?GGñª?õ?:´pnÉø?ïú.•~p?:´pnÉø?q™¸Ö-{R?xúŠwr|"?ïÜ̎S¥
?xúŠwr|ƒ?…Œh5ÑK±?s)6Î樓?ï©Î_(ºÑ?s)6Î標>h*ܙH¢ý>j	l܃Å?ïÿÿçÕ#f>j	l܃Ä4FGL J1627.7+3219¿í,âáY@EžNaŒâÒÀ:ePÏ%l¡À<»kõò`@1ONFßã?ú¬d\ êÇ?Æn¢ŸýŒ?äv‡*¯@Ì ~$É
?þô¿ÍŠâÈ¿å<ççÛF¿ÛЏ$Äì¿Dr}Ëݹ"¿äج¿f1ã¿ïÿÿ" 5•?ïÿ̾ßú&PSRpsr3FGL J1627.8+3217PSR J1627+3219?8óíCMÇ?¨g[0ə¿?ï8`•å'?¨g[0ə¿?§mewø?²†Èfq Œ?î‰(	¨€}?²†Èfq Œ?À_Â¯w
?ªƒXØMÿ?ëèT">?ªƒXØN?­·µ~­«â?¡Â<Âh'?î$"¨%A?¡Â<Âh'4FGL J1628.1-3204¿Ó).ºåÌ@&ûžŒG¡À9>	 '²À<OB]r¢@ú=ºË˜@_'c3?´S~¾].•?ÞÏ·£Dé@!h0Â?«?ögR]šæ?ïôî<‰¿ÙÕRAì3š¿ÝÂž»¿è˜f~9@é¿îÍê¿&¿ïóêþ'PSRPSR3FGL J1628.0-3203PSR J1628-3205?DÏà_ɉÇ?>:?Œ­?ïúÌè
ž?>:?Œ­?s_Q—ë÷?:×`²F{?ïÙAñ\Ð)?:×`²F{?‡ò'Ï`T?l"ò†Ë?ï 7`ÂÎ?l"ò†Ë;?
ŽþR'4]>ü<j¢ª•?ïÿ•Äµ¸>ü<j¢ª•4FGL J1630.6+3734¿ëª³@Ešgó
NÀ9ØScTc/À<OÓ7ë)@(¡Ê?©¹?þ"•üV'?¹5Rr=µ?åR›¾aúò@Ì­~«@Oú)ƒ\?ïĬ½bÌ~¿ÖN¾ÿږ9¿ÓÖ¢¤V§¿åˆs¡¸L¿ïÿ÷Ò4Û?ìDÇ_¥'PSRPSR3FGL J1630.2+3733PSR J1630+3734?jÒîL¿Ú?oª¹µÒèœ?ïåï-³??oª¹µÒè›?•=Ôj":?™AÁƒyOu?ïV\«f/?™AÁƒyOu?—ïMÑèÁ?Š#ú"??ïGЅ'pº?Š#ú"??uk¦_{¸?ißsBÅ?ïÕ(³AÍ	?ißsBÅ4FGL J1634.7+0235?ëOdÆs½'@?T›«–òÀ;p>Ȓ«iÀ=8؆>s@I á÷×=?ÿîóhB¹?Ô¡…‹Å›€?ïüÌnØû¯@(™|=h?øš€Y¦‰?´/ȀÈùj?î$¡ÿ?×ÐÇãÙÙ¦¿æµ¹?§4ã¿ïÿý±q&´?ïÉ+ø¬N¨PSRpsrPSR J1634+02?ÉAxìV¤?Èdggzâ?鯡Äê~×?Èdggzâ?¸ì.	¤ÿ¿?Ç°˜Ê%&?ìâz>Ë`	?Ç°˜Ê%&?Ó05‹í_?¾cA±®y—?ægå:	P:?¾cA±®y•?'€œŸ¡ã.?ŠûÊgòÁ"?ïkûðç?ŠûÊgòÁ"4FGL J1640.1+2222¿ï'Ö!Ñ}@C&³÷+EÀ:É[ÇÎ`À<©'¿9@æ!ƒˆ`6@Úmý3œå?ÆR6X¬"s?Ýd)uDP@úÃ")´@¾OhÈì¿¿ª›©ä@?ïóŠ¦·¿Õ­N ¿ã‡ÕÍÛ@¿ïþg¿Víx¿ã_Ř%%SPSRPSRPSR J1640+2224?¨.2ÌeÞä?¥Ñ¿2ÅbE?î}Ó9¢?¥Ñ¿2ÅbE?¾ýw<pŠy?Ç–¥¹ï=?ì Qqî±?Ç–¥¹ï=?¶ƒ¿wj?¤ +ðª¸?í/ˆ?¤ +ðªº?½µÃª|?¢HlLës?ì\©M犱?¢HlLës4FGL J1641.2+8049?çŽxݘÚÌ@?ij=¯øÀ:Ôcb¥ç†À=f{_ï@ªž+#Å,@O–ü0g§?Â;¶šM?Þj'Ûdj8@°4ß۝J?õ;qE< ?ì?i¢[?î§À&KC¿Ý¡<é?t¿è®JáO»ª¿é¨äÅçÖ>¿ïýªë&PSRPSR3FGL J1642.4+8045PSR J1641+8049?ÄtF]ÃÇ?®@Îöô­'?ï€î.æˆñ?®@Îöô­'?­F|
?½J‡N¨×¾?î+˜>o'è?½J‡N¨×¾?į–¯Ó1?¬Gy¢'''?êÔ>šT4?¬Gy¢''Ž?}àÓÐ?jDMçÛ?ïÅÂx¾YÌ?jDMçÛ4FGL J1641.2-5317?ÈõªÒÀ?\¯-•À8˳;+À;TÚÌiÐ~@=³é@åŸ+©Ò?³²¹¿î†Ë?Üe;µg@"n½	á*R?ÿn±†uO?ïîºþn/‰¿ÔDûb6¿â¦KÄ#°ß¿éKF¿Ä§¿ïýu@ô¼Ö?ïy§4ƒ?PSRPSR3FGL J1641.5-5319PSR J1641-5317?Š"&	'O®?'>Êø×ì–?ï—wgÙºÀ?'>Êø×ì–?"¨9–QQ?¶@Ó"?sÏ?ïb¿f3Mv?¶@Ó"?sÏ?š©´‡ýÃ?'Å=D_Ú?ï/b²[À?'Å=D_×?@äêážøç?9>^V.?ïûÆÅG˜A?9>^V.4FGL J1648.4-4611?林gä¿éÏ]Àû]YÀ7ÄfUŸnÆÀ:b¸[ü€@ 1)ÆMå@£¢Y[»è?°áà°.†{?Þ9ÚÙ)ý@$ê ¼8*@pjKM[?èY}êçj¿àÌö¡¿Ë¥ô[\6¿áڕwËéx¿ëbšÿË&Ú¿ëDLˊ­nPSRPSR3FGL J1648.3-4611PSR J1648-4611?vKŽ…þf/?­Æqú·€Ð?ïÓhâô3?­Æqú·€Ñ?`³ÚÀ«]
?gËH""	?ïïL%?T¢?gËH""	?™èÇõÐʳ?'0E|"Ì?ï0¹ÀQyª?'0E|"Ï>ø"@ð͙m>òÐÛ½:˜#?ïÿÎÙ~d>òÐÛ½:˜#4FGL J1649.8-3010?ï¾¾ì«Ìƒ@"lQ¹07ÖÀ9`òl™†NÀ;ë]"ðÅÐ@I í¶Q@§ºÄŒŒk?¹"ù¼o?ݞPõùl@ ™÷L¿éñ8ŸXËH?ï¢ý$ƒm¿ãÑàd)u¿ÚºûéðÊ¿ã@Bæ.ž¿ïÿþˆ0»Š¿ë·é íö¾PSRpsr3FGL J1649.6-3007PSR J1649-3012?´5ç²	ü€?ÇÅåŧ-§?íyC	¾Àq?ÇÅåŧ-¦?ƒ¨Øˆ"SK?¥aH{Öá»?ï±\Ýîµ?¥aH{Öá»?°ÔÁW{oŽ?¡¢¥ë?íågÕ'?¡¢¥ë>½FkŒ>·K'ØBL?ïÿü\Í÷3>·K'ØBL4FGL J1650.3-4600?ìÝÕÜyX¿î€ž@GmÓÀ7¬r•;fÀ:GÏASC@80Fé@bO̲+?²N×>ã'?ÞÁ»=j@&–V«Þ?¼@RÞ³T*Ð?ÜÇ<? |L?Ë¥ñÁ£ÎÒ¿à4äv]¿å½‹±yŠ0¿îø/¼†-¬¿éœŽ i¬íPSRPSR3FGL J1650.3-4600PSR J1650-4601?R)‰'7W·?‹d+fµ]?ïöë;6äR?‹d+fµ]?XØÄx²4?dÅÈ?ÔÖ?ïóúÃ¦?dÅÈ?ÔÖ?'bލP®"?\Sœ¨+Ó?ï¶t…ʽH?\Sœ¨+í>¼µ¯­'b>´dFü§'?ïÿüiJ
_>´dFü§'4FGL J1653.6-0158¿ãÀâÍu©á@8ñˆÁÛCÀ8Yˆ1'IÀ;ˆ×§b\@ÕºǬ@‹ôÄü?¤gÉ<õSÕ?Ñí×ßO†P@+ÂÑ(| @Åìäo"?™žõµ5¿ÕÀáÜÿIø¿â£ÿYçÓ¿ç÷Í+—]¿î¢Î–Ñh=¿ïþ'MKã-PSRPSR3FGL J1653.6-0158PSR J1653-0158?VQ•p4ïø?Mˎð$ŠB?ïô×5Gå‰?Mˎð$ŠD?oIn!`ˆ?x‰l·ù²?ïඑýޟ?x‰l·ù³?—€8[¥å?ÚGüP??ïCþ?U"Ò?ÚGüP>>â"ùÌr½á>ß°ì¼°?¹?ïÿíÝ3Ž>ß°ì¼°?¹4FGL J1658.6-5323¿ÒGm3£MþÀv/¾3¬ÖÀ8¥èYM‰À;š
oTK²@$$5>{@<§…ëfì?®¢Ç{æ;š?àæ
Î&"@)¨U•:@u—†ÄÖ¿Ó¼¢}méè?¨­1žU™¿ãaΆá01¿ê¥)Ô½\¿ïÿ÷fÔJp?¡j£	#PSRPSR3FGL J1658.4-5323PSR J1658-5324?Œ%w˕?°k.]v$4?j Ñ­?°k.]v$4?u0ä¿FlÃ?'/Ãa"Ÿ]?ï՞6s'?'/Ãa"Ÿ]?™½.N8?r[ï<?ï2&‹—?r[ï>>ñ9Э#À>è³G6V|›?ïÿ݌^¥¹>è³G6V|›4FGL J1702.9-4131?äíYÒnŒ?´Ûö5{âÏÀ8t™ŸxÖ«À:=
:{&@vRëŠR)@Æ
c0Q?Ãӑ·øÕ>?á=;•"d@·²ôݍ?þn©›z?£‰£édï?ï ^¿Óêù¿Ý·âYü˘¿ê‰œ*Œñ¿ïÿ§J\D¤?ïïùø?PSRPSRPSR J1702-4128?Ô7}ã#?٘d{?åäAyüo?٘d{Ž?'gÑoÈâ_?¦"Ïa=?ïlÁt¸ì?¦"Ïa=?°oü^rmÃ?¦^´»X"Q?íòt1²H?¦^´»X"Q?;ؗ="0V?4†=×iƒ?ïü"íMz?4†=×iƒ'4FGL J1705.6-1909¿ïÿþ :õÓ@)ý‡ÂÁÀ:7/p0ÄÀ<O!Æ#e`@ÌiiP@;ªe™·Í?α%|fWù?ïþx
Ә™@媴ts?ùùu$dÖ?ïòù¢í]?×S"ÜùÀ¡¿âànrb¿ëå#¿¸è¿ê^ëÈRj¿ïÿYM»PSRPSRPSR J1705-1906?ÂŒIñg™?›å¶C8¦?ïy띰tÄ?›å¶C8¦?ˆBÂ;<ò?'YCc)CÛ?ô÷?'YCc)CÛ?¸Þg€x'B?£åƘVy²?ìä3ðï·?£åƘVy²?9Iu±ª/?(±RºÏ?ïüÖÑ\‰Ë?(±RºÏ4FGL J1709.7-4429¿é-hH"À~DÄU/À4h1†:À9qŒ;E‰@&ôî)ô@ÚZæÖc?y5£ •?ÑyQ…XÄè@T8sWæpã@†MZý?¿Q~wÕ$¿Ð›YÂéôü¿ßt†¥ 5€¿ãáû2:寿ë£Q^‹³¿îs'i#°PSRPSR3FGL J1709.7-4429PSR J1709-4429?K]ö2òó?DI)jñV€?ïù('sCC?DI)jñV€?8c8³aÈ`?SI Ár»k?ïüó˜é"Æ?SI Ár»k?ƒÚ4"Ë»š?j=h/™?ﰗ-ìÑ?j=h/™?ð4FGL J1713.8+0747¿ì[@LøÞ@95Ïþ°t§À9­¯j¼6}À<9HW‡¦R@"»ß@î?ý@YŒcP?·"~ޓ"é?á<ñvu¨@ Áòº`@NJƒ&:§?îpOô4ã?¿'ð]À»¿Ä£Ï½íáÅ¿âí ßôq׿îúS] ;¿ïú­z÷íãPSRPSR3FGL J1714.0+0748PSR J1713+0747?JÐÓþ?=>6ã0x?ïù\ùË<?=>6ã0x?}3cÐ,†Ù?æXEy0O?ïř8_¦ó?æXEy0O?‡–iz†Ú´?hbw¿ý¼?Zä•?hbw¿ý»ø?V…Eَ?GÃGҏFÝ?ïô½t]q"?GÃGҏFÝ4FGL J1714.4-3830¿îã[T……†?¾óÙ@£‰2À7_Ÿ¢ÈÀ9¿¬aó:@ –lŠÂ¼(@"=ÚV"L?¬÷ÃhcÛ?Ç1Ubˆ
{@¡\Á¡ö_?ú|ePç¤?ïééªS%¿ÚŒÉÝ.Cà¿áŸ—£ö¿åô¯iå¿é+܂!'Ý¿ç×ó;Ì^éPSRPSR2FGL J1714.5-3829PSR J1714-3830?gØ3ÚT:?s$}«ÒYM?ïè'Ì%«Ç?s$}«ÒYM?j:*ûÀí?s
bä™.?ïåÅÕ÷@?s
bä™.?Èԍndœ?´Ç.â}ÐÎ?éÊܤy¦Ù?´Ç.â}ÐÍ?"Þnf
«>ýe^é
š?ïÿ«t†Fh>ýe^é
™4FGL J1718.2-3825¿ï*c‹€»à¿ÜH%EáÀ7	hQ"1ƒÀ:0«¼²@'ã»-h@ÎåD'×?¦(Öbø¶?ÖÃê¥û¨@-Tšþ§±?ñü^]-'š?ïš ri¿×Ÿ2à§õþ¿ä± Hõ½¿ç+
=²é¿îFY¶T»C¿îNõѨԠPSRPSR3FGL J1718.1-3825PSR J1718-3825?‡lcÝ#&?µˆÛšÌ?ï¡ÊNp‹s?µˆÛšÌ?QòŽà?]Ò®ïÏ?ï÷?¸ð?]Ò®ïÏ?ˆùûÒ&O?zD̙j+ò?gƒ?zD̙j,>9B®Y>@@X¯-£?ïÿÿü×½Î>@@X¯-£4FGL J1720.8-1937?º¸³ål‹@#‡ÔCédÀ:!4AP,hÀ;´%ï@zîüÍpŒ@ÏBBš¯C?ÊËúêÂV?¾Ê°'Úb¸?÷â™7t
"@¾P7¥Þ¡?ïü6¢(‰a?Ë^7u¦¿êR®ž8¾¿Û`·õ¥3¿æñX½†]Ó¿ïõ=~æìPSRpsrPSR J1721-1936?ï̶¬8?"Á4r0œ?yý~$©ã"?"Á4r0?ïßC«¶?‹2õ‡f?p^*r$¤?‹2õ‡f?îȳvîé…?˜Á¬Àа9?£tȑg˜?˜Á¬Àа<?î$ÔüCg?'«xcQd—?­²°>ûɕ?'«xcQd–4FGL J1728.1-1610¿è˜²è‰m-@$`;ÄÒ,ˆÀ:S'ŠŸbÀ;ðaXàkæ@³àúVGà@ê%Ðt!?×0y@?å¨Íê>y@/À_A?þ—ÌLÊ3?ØwGà{ˆ?ïôà²\Þþ¿Ä
8èÿ³T¿çÙÁ§Õœ¿ïÿûbâMh?ïÿ<Uñ¤PSRpsrPSR J1727-1609?‡u€ë¬ß#?•2=âAæ?ï¢)üQL"?•2=âAæ?£¸üGèßÃ?²Óhí´ú?îÄp;r?²Óhí´ú?Ç%i4ÍA?­îæ]¥#¦?ê6¥¿2Ì°?­îæ]¥#¦?{Ÿ^?=á2?p*©eK?ïÈÁC"=?p*©eK4FGL J1730.5-3352¿äßø>ý|?°ÎÃG
IÀ7⺎ç¡À9Ú׊•ð˜@j±UXL@½ÀÛ'£?¾»+ÿQC?Ò܌=:ž@<ewS@H)Âq)8?îúæ ³iN¿ã5'»0¿åÞv½÷qç¿éª<P¿ê‡¡8¿ïõ|RÆPSRPSR2FGL J1730.5-3350PSR J1730-3350?°;#ó_z?ÇÏP†´?íø›Ÿ"?ÇÏP†´?'=ÖÍJ–y?¤Ç|4›€õ?ïvI•«L?¤Ç|4›€õ?´+ƒãŒ—þ?¥ÄÛÀ?ízƒŽlÿ?¥ÄÛÃ?Tã}'ZNp?D3` n?ïõŽAlRÙ?D3` o4FGL J1730.8-2303¿ïî—ó¸J™@ÇŸ¾vÉÀ9£@4£vÀ;AÜ@W@†ž^ÐDü@(3àØŒ?ÉÓËñÛz?áRíãÉª@;ç)oe@yÙú1ßÌ?ïItR¸3¹?ïÚyޓHÈ¿ä3ÞSÝοë
`z"¿ïþBžHU¿ïøT¥sÂoPSRPSRPSR J1730-2304?®2F•Fµû?¿`¯!Òk?îۖ«"¢?¿`¯!Òl?Öm«uò?¡»˜¤V1Ë?ïyL"z¤Q?¡»˜¤V1Ì?²ÚY¡=ë?¡6:,p{?í¤´ËÜXC?¡6:,py?t"®gvp?f=k1•z?ïÖ×Ä£1?f=k1•z4FGL J1731.7-1850?éüýíg~@ ÂÀð À:;ô¢ÕÀ;ÐÔÚ¸GÛ@öÀ l8@­±™jŸ±?ÎðʐÀW?æ¿Û¢¨‹û@­¢™ó\@(ÿ#·T?ïõ桊(ã¿ââ÷Fÿä6"¡¸!¿íÅWïnb¿î¬ ‡t~¿ïPk®ŒpPSRpsrPSR J1731-1847?½…yªBBø?Á!;CåvÂ?ìOPÊ··¡?Á!;CåvÂ?Ãp‰W?ÊMýÄCÎ?ë#ùzª=?ÊMýÄCÏ?ÏY·xgãÖ?²-×34M?è)'!æ?²-×34N?» 5ä{? mؗ'}?읻ùC|1? mؗ'}4FGL J1732.5-3131¿Ð5°œzïö?ðã†Lµ»À6ioê›ëÀ:oE	@OÁ^Z@|¢}méè?˜‰:%ë¢?ã/џ‹A@A㦽nŠø?ûȚ$W"?ïáKª"}Ù?Ðxoþ?¶y¿ÑZ³ɹȿãÔÐ=0ã¿î.Ö­ _¿îË¥»PSRPSR3FGL J1732.5-3130PSR J1732-3131?-ïI·}?Jî2uý
V?ïþ!d‡?Jî2uý
X?DOE°êlŒ?ZKOeÓ,ÿ?ïúì."Åe?ZKOeÓ-?ø¥Ïn7å?V½"¢{Q?ï¸hÂG?V½"¢{s<¡D®ÔJíE<Ç-Ñìô$?ð<Ǔ܁ye54FGL J1732.7-5050?è6jÁ 
vÀ"énX£/EÀ9×ò<ÉÀ<2³àl¼Â@·(@7`9%»{?»UJ	c?Ôßs㧄¿@¢;ÿŠ@ôöw5F?ïø€_5ð}?—Ä֚g¿Þ|RáÏ=j¿ã®ŠÂfA}¿ï7iÃèø|¿œ}ãä*ÁPSRPSR3FGL J1732.5-5048PSR J1732-5049?ÓG›}?Ƃíí­:?æ\sz|2B?Ƃíí­:?Õtº‰­ö?ÓӖ§ŠÞd?åE¢õ;)?ÓӖ§ŠÞd?Î> 3´ée?´2€½	­?èpWóÅ¥?´2€½	­?Üa£ˆˆö?µ°öÈq9T?áÏ.;ó;"?µ°öÈq9T4FGL J1739.4-3015?ïü¤#ñ?Üã!M»À8¤i×4/À:†ð¬¥åØ@øèë¡@âEõ­–§?Ä_|sp?ä÷—{²(@¿ï|$=Í@nCG'†Ø¿ïЅžºë¤?ïüúz…¿Ù#faˆÜ¿ê@þB:¸
¿í¸^_Ö¿ïÿì´É ÈPSRPSRPSR J1739-3023?¾(ˆ£WaØ?ÑږuŸ¥¾?ì:îë•Ä?ÑږuŸ¥½?"ßãD™K?¢ ²(`?ffrïåš?¢ ²(_?¶Õ¯Íô©F?§0ytÊW?í%JAjØ?§0ytÊW?Sc©#êü?E|&,/ÌÓ?ïöNv+n?E|&,/ÌÔ4FGL J1740.5+1005¿íPœqÈÕ@4EèÄzôÀ:ý©äjxÀ;ص–Ob>@Ìò"l`Ñ@"à??Æj©V¥ÿ?ÉF…àÕt?ú˜äÓSϋ?ücñ9Æ+?ïýÞ½ç¿åԅ=l3¿ìÊAR¿â&H3uxR¿ïútpe¿ïŽhþÇÜPSRPSRPSR J1740+1000?ïÉ[ÄÚ*?€ë(?ýHZ?{RÀêí?€ë(?ýHY?æú'Í0.j?Ð(@‡RaÄ?Ò°eŸ£*?Ð(@‡RaÄ?ë!æ?­'sø?Ãß{·"ìg?­'sø?ä/÷Uá{?·ƒOihͳ?× T=	ð?·ƒOihͳ4FGL J1741.4+1354?ï.@3œÐ@5«ä›«—À:5òý¸ýãÀ<O)õœÏ¯@å7¿)Ì?ÿ±a‡"à?Á¥[Ä¡Û?Ü	`{ë´@ .s±?þ©l$ìH"¿Í®Ñd65q¿à³xgðª¿Ò3Ðý^*¿åIåý{¿ìË`P¢¯Ã¿ïÿê0ŠâGPSRPSR3FGL J1741.5+1351PSR J1741+1351?¡Õ뛛?Ÿ2l"rø?îïâ¯ÑFF?Ÿ2l"rù?£zJ§?°Æ¦áº?îÈW^Ÿõ?°Æ¦áº?£w+‹ý(?šcQñjM?îȎÝG@.?šcQñjS?¾61y‰X°?¤»‰Ÿu%?ì99ÐÎÔê?¤»‰Ÿu%4FGL J1741.9-2054?ﬤßX	@Ÿ@=ݱ!À6äN¼üÀ:Á±RóÂÛ@%'cœ1¤@)õ>ÛÝâ?š¢x²¼?è
U¾xv3@C¿ohی?þa3™Š€!?íúՉ3ðÈ¿Ì8èê9Å¿âOÅÀi<¿íu!À5¿ïÿ¹žœ¸³¿ïÝ6LJ[PSRPSR3FGL J1741.9-2054PSR J1741-2054?|ÁÚüø­ï?¢¤}3á¬?ïÆ|J¥?¢¤}3áª?I–œh@"?c-·A÷R?ïùšXýåò?c-·A÷R? éhË -?•0ªxœ	Í?îñisMý.?•0ªxœ	Ë<‡<¦ý£
d<ÁgœmNk<?ð<Áw‰îL4FGL J1742.3-3318¿ã¼hÈ{ÿ¿ûÚà‹ÆrÀ8ÜkÝËùÀ;/:Wꢡ@ŝ7³Ët@tEêPk?Â|˜1º?âú'
‹þ@–¿Ê…Ë?þ=šOw¥¿ê}©Æ˜?
Gç¿×!³ƒûw°¿æhwM>w4¿ímpEã9 ¿ë&€IRPSRPSR2FGL J1742.5-3323PSR J1742-3321?;Rrù=S?7º‰_ÅÎ?ïü•¿Q Ù?7º‰_ÅÎ?"Iñÿ/?¬ýŽÆŒ{?ïe·xp'?¬ýŽÆŒ|?ˆÏZ"»?l›$KÁýM?Ãƕ°?l›$KÁýD?FÁ—pß?2"¨ãZ6?ïúOœ;¤?2"¨ãZ64FGL J1744.0-7618¿ïpñ•BJÀ6t¾ÆyÌuÀ8¦-vZÐ0À<óý">6@˜rÆñìl?ü̲{ï?¨4_>e&²?ã8MžïCð@3Ö}sÉ?ü'@³½?í¸Á>#Q?ÔY3wü'¿ÕfŸÜ©¹¢¿åü­_I<¿ï¡±Ë¿†"¿ïüûÔ!TäPSRPSR3FGL J1744.1-7619PSR J1744-7619?VT[éç9?Sü'Ÿ‡y‰?ïôÕöÒ?Sü'Ÿ‡y‰?x"\֑Od?‡QFöqÙ?ïÎ÷FRÝ`?‡QFöqÙ?ƒÿ£4¢O³?\þárbs(?ï°s-vÀ?\þárbsF>5ØgUU>; *Up?ïÿÿýDÿ'>; *Up4FGL J1744.4-1135¿ãR,þ7f6@"]·k;¸=À8r¥®À;T¨ŸÆÚE@¾õɛ?@õ\Rç-¡?§G3¾/?䦏ãW@3áœàu÷@蕫"ƒ?ïþ™côÏ¿·üæÅò=¿à-1üÒN¿êꛟƒ=¿ï×ßÖjÛ¿ï÷ß4®]vPSRPSR3FGL J1744.5-1133PSR J1744-1134?i!N¢C"?hµÇ³ó%?ïæÞþ±]½?hµÇ³ó%?gõPÕdùÔ?'l¬fô?ïè
¯*›?'l¬fô?ù¿#d—®?…§¨|#;º?ïx2äÛA?…§¨|#;Á>¡lqüC>*›++˜g
?ïÿÿÿôŸ>*›++˜g
4FGL J1745.5+1017¿îs^Vpþ†@3>­-ËfÀ9šVÿÁßÀ< W¯ê=÷@VWwá
!?ÿFôæÇIÖ?¹=uai|?àE=V¢¤@ 'ÛçòÃ?ùð:æ?â'!,öX¿ÜX°»t4ۿӍÈhûí¿âä
k"ÌÑ¿ïÉûa4Î>¿ïÿH˒:PSRPSR3FGL J1745.5+1017PSR J1745+1017?]@µ[öó?Uø¦#är¸?ïñ_¥Rú?Uø¦#är¸?y(€âwÚ?ƒ""ôOܺ?ïÍ®þ;L?ƒ""ôOܺ?œ+U<–?€x˜'«÷?ïÃ¥V?€x˜'«õ?E_Ž[Q~x?4#ìÓ$–Ô?ïú¨i+¡?4#ìÓ$–Õ4FGL J1746.8-3239?×öb›X€#ÀY1¢9{LÀ7Ãu"*ÐÀ:ïoɼw@M,…šT@o<¥¢¼?°süPH?àÿ»lR8²@0¾ß¤@?÷ ÌäIÁ?ïë)yv
£?è)8Þm߿ݸõ_='S¿æ°ô>«·S¿îw.4Ʊ*¿ëˆª"¼àÆPSRPSR3FGL J1746.8-3240PSR J1746-3239?7H	À{÷Ë?7é{´íÎO?ïýþÇð?7é{´íÎP?XŸ¶XJ?o"îÈa?ïó±0$ÓÜ?o"îÈ`?'õ¹ƒ"?^LŠ¡¡o?﷜)½ñ?^LŠ¡¡€>0f¤³Vþ>4""nÖ¾)?ïÿÿýó+k>4""nÖ¾,4FGL J1747.2-2957?Ù
ŒÍTâ¿ë
ßòC~ÛÀ6'Ôº××ÃÀ9½åëoO@ÚÙÇ1@Åûø3ƒ?¤RRá#q?Ø^TùM@0yJ€à@eݶ•?çS¼_í%ˆ¿Ô¼"E$Lf¿äjšêÒq¿è'kí"¿îCƒbu–¿ìùÍ¡^	 PSRPSR3FGL J1747.2-2958PSR J1747-2958?Sõ*ÞX
a?TˆðNGè?ïöjÓû?TˆðNGç?Pƹb}‡k?]>RUwNa?ï÷œ£NÁ<?]>RUwNa?—8é_â¸ò?"ÁŠ4™ª?ïF8µê9?"ÁŠ4™ª">^þ°úúû>cµ¾vYD?ïÿÿðÀ§>cµ¾vYC4FGL J1747.7-4037¿¶Û,™¥J[À¥P"WBÝÀ9"A!"µÀ;ϜÈù¶@,ØCxz»@ŠwTË?´–Õ™úèi?ܘÞ]ÃՂ@"'6¬dwy?ÿü¨G1lß?ïÉ%x_.¿Ûz1¿•¬¥¿ãFÓ#(#¿æ£»-h¿íœ=þ"Ci¿ïüe¬,CUPSRPSR3FGL J1747.6-4037PSR J1747-4036?K'=ØZƒ?FÆ"H®"R?ïùp‰é`?FÆ"H®"R?~îÃÉÜ-'?…‡4£ø{Õ?ïÂ"xlG¥?…‡4£ø{Õ?'3U¢»½±?'–ÜŨ5U?ïveRê"?'–ÜŨ5Z?'3Qœ¨"?¹Ü?ïþŒÊæ>æ?¹Ü4FGL J1757.9-2419?㏚µd9¿˜K?™s-À8xh¶¢¾ÜÀ9ø#CÑæè@ 4ÇÞ%²@«¨?ùA7Ì¿a?ɳ‡i!,@S™ V¸@d¡¼'ãõ¿¶ÍgÑöW?í»
bY'l¿çæ a3÷¿ê^˜q{m_¿é*qš!¿Ð1Ácb%PSRPSRPSR J1757-2421?Áò4\±Ç?Ê°@hŽŸt?ëƒrèÓ¸?Ê°@hŽŸt?Åö{& Hô?Ðßöy22?ê'a6wíÄ?Ðßöy22?ÕEOÚ?¹±…ŸžO¼?å]Xtpp"?¹±…ŸžO»?Ö22YÈ,?ËJm|=ù"?äæôæÓê?ËJm|=ù"4FGL J1801.2-2450?áŒõ±Ñ¥z¿íÔPXÝèÀ82ÿݛQ*À:šÂn¤ù@=öÔ{@B­Yiþ¡?µÚÎ~cïO?ÎÄ»Ü9§A@>¢Òþ??õåC¼s?íÈDÝ¢x¿ßÆ:ÂÇ;¿áõDD¿ä¿T_™¿é…¡—û¿ïÿ&PÌ¡.PSRPSRPSR J1801-2451?hàøt'éÀ?h9?EC{ë?ïç‹n?h9?EC{ì?‹8ëг?—U,ý˜éæ?ï"P½1Ë?—U,ý˜éæ?¹DSû#ˆ?¨/"=ÊV,?ì×u€ž?¨/"=ÊV,?>?"Ìè`?.j›eµ?ïü/Ø
†b?.j›eµ4FGL J1801.6-1418¿ÖðW(JK@Äk¬÷DpÀ9ß%"åÀ;ÕWµÉ{@Ə§þ6Q@3ƒB??±?Лl¢À‰È?ä›@ãŸø@kf¶~¢@_s"\³?íYiþ¡[/¿¾ò\=îx¿ê5ŽøU瓿î],áŠt
¿»ÂÚô¿ïÿðÇô PSRpsrPSR J1801-1417?Övи^6?Ðyîx?t¼?äė£Ðäò?Ðyîx?t¼?É°R){-?Ð݂Ö^j?é"ëyµ¡5?Ð݂Ö^j?Ýʬ<tx?½Ç·7.,?á©áÅÃõ?½Ç·7.,?Í#"Fð?ÆÜ×÷aF?è¸÷=÷nD?ÆÜ×÷aF4FGL J1802.8-4719?ïÿî'ÛmÀ(qûÅޜÀ:šÉÓIÀ<2w¬ßÇ{@ÃßóE1@@˜ü»§á?Оˆ@Ö´Ø?â9Ž—@§ôÛߏG@؟ÎçÚ?ïy ÕÍýN?ϳù—02οâ¡sîeô¿éÅ# ™5¿íŽÁ.32¿ïþ"ÐÜýPSRpsrPSR J1802-47?ç‡>õY˜?ʛŽdڃ`?ÐñƒÜLÐ?ʛŽdڃa?Ԝ*1¢:?Ð\n¨ül?å±êç.Àc?Ð\n¨ül?ÜÞ;HVñ?¿NB
' ?áâ[ԇ}?¿NB
' ?Ä7—ƒ=ü?§=¡~Dò2?êò;0€?§=¡~Dò24FGL J1803.1-2148¿Òzª©Âá2?Éx.û@'¸À7"èG|–TÀ:´v"±Ó@çûZ(ë\@µô^N?¦X"Ãs³?ÑÑ	\õúC@%DæŠ
5@½í;WD
?ì­nB}Óë?îè* dú¿à;­àÎaw¿ãˆP›ùÆ*¿ë˜K$Á€¿ëõe<š»PSRPSR3FGL J1803.1-2147PSR J1803-2149?-•M´é€)?3¸™A"?ïþ&«$±i?3¸™A"?TžFg-?_ÌÒ¥ZFT?ïõ°ôÜÌi?_ÌÒ¥ZFT?ƒ±²u:r?hG˜U7?ï±;á6+?hG˜UV>ÚMèžÅÝû>ӇKX®C?ïÿòÙ°œ>ӇKX®C4FGL J1803.2+1402¿ì%!‹[@0êkƒÙ^À:˜û܄еÀ<[›]@@Ìxé÷@Ò¶»éOº?Çâ·ðœ¶?ۘjû .@Eâb`Gh?ö±Ûø8áH¿àfç?¿³Š?tÈT0󁱿á¼v¾MX#¿äHb°Ï@¿ï²äXڌ©?ã÷äþqàmPSRpsrPSR J1803+1358? ²ðG¢J?ž¸¥"€Ñ?îþDÐû…Û?ž¸¥"€Ò?Î¥3Ìj?э9vå?èV³û:æ?э9vå?ÁÑGÄO?³AŽÅ?ë¿<K®ì?³AŽÅ?Áa‰/Ç}x?©ûÎcK"?망´ ¢?©ûÎcK"4FGL J1805.6+0615¿ÖÂÓºRq@*΅3±À9öÝpˆÿÀ<1#|
Ü@Þ~Û¨1ã@"à¤ðæ?Áw'iP{˜?à"<›<@#VSÉ«°@ßT¼oÝ^?ïâp"&ñ[?ÀÏÅ0¡¿Óª;½ÆI¦¿à눯fŠy¿ïÿ©-‹S†¿í£?O¦†PSRPSR3FGL J1805.9+0614PSR J1805+0615?²éÈçÔ?ËîXUŒ³,?í¿ÂÆãf?ËîXUŒ³,?‰ ]Ú¹n?"Ð[æ/?ˆ•?"Ð[æ/?"É´úùH?'
WZɔ?ïa²X(5¿?'
WZɍ?™¶Á]H¨?~7œŸ.9?ï7zIõº?~7œŸ.94FGL J1807.1+2822¿Ëú†L"@5‡,ƒì‰+À:£àyQûÀ<2È b@4÷â¥&@á'©?͵ûåi%Þ?Ê®¢jM¦§?ú†¦\ö{?ó™–dïï?âqíþ ¯c?íØ涂޿é8h\	ì¿ë(0Àè#¿Ç°I‰`çK¿ïÿb¶®}VPSRpsrPSR J1806+2819?ïÄ¿ˆf°û??¶Š
Á?} ;̧ƒ/??¶Š
Á?ê3<@I6?˯²€©?Ç3þÛ'™?˯²€©?íK
ý9ʱ? ßIªHEt?µ§¨1ªo? ßIªHEs?åÈý´LËê?ÀüP"ò"œ?Ôn—fh,?ÀüP"ò"œ4FGL J1809.8-2332?ܖeãAÿÿóÔ
2îjÀ5˜µnvÀ9²æ[L@ÔQÞÄñâ@ܕà•×?½ÅüV±?ÕÕØ#ÂýÁ@F-¯ ê[S@''[²ƒJ?ç´4ºò¯µ¿Ïñ¤ƒ³ÿ¿àÞ°z¿äé^¾Q^í¿ì¶óé	¿íI³bmˆoPSRPSR3FGL J1809.8-2332PSR J1809-2332?6Ùö"à£.?+œUøüŠ?ïý$Á-ƒì?+œUøüŠ?FpZ¼';¼?aØ-v«-w?ïúcéPö1?aØ-v«-w?í´Ÿ+–?WæÃ'1°?ï¸I-ƒQ¨?WæÃ'1ç?ð4FGL J1810.5+1744?éCr2¡Oè@0ÏîÑížÀ8(Àéi¼À;›I²Ñy@fúÅX8@Øu'ST;?§L&Ÿ& {?҆µ¼:…@%p÷…@ÖoºÜµ?ì÷ì5Gài¿Üd…üðJ¿ãÌ©C6Œ¿èä"ŸR¹¿ìô#ˆ›D•¿ïó!3FPSRPSR3FGL J1810.5+1743PSR J1810+1744?e¤ç%¢ÄX?aÂtèäÊï?ïê[Ú];?aÂtèäÊï?r!NªYŽÌ?|XǾÍT?ïÛ½b«Lã?|XǾÍU?«Ú7T$¨?¡'p*èoï?îO'\Š½¶?¡'p*èoò?4ä×TÈÐó?+"%ã8âC?ïýcefæ?+"%ã8âC4FGL J1811.3-2403?åÚ¯TF¡¾ÀWg?ª9ûÀ8µml%QÀ:'
©§-×@ ?z¿8å@{Ú¡¡¥Ø?Âü$©,µ?DZéDŽc|@±B³÷+?ínÀ	šÞh¿îÌÂn¤ù?êðL-Õü ¿àÞ	|¿æ°¸.°´¿è‹X=®·8¿êGM1:ÇPSRPSRPSR J1811-2405?ÌÃu0–J?Ò\'Žg¯¿?èÿ"³Ún?Ò\'Žg¯¿?Ð}Y1p?ÒUýç®çl?çÁSgG¿9?ÒUýç®çl?ÒîÔ©´=
?¹}]/©#~?戕«%á{?¹}]/©#~?'¹®
4M?vzo&ù?ï·õG×.?vzo&ù4FGL J1811.5-1925?È$OÜ@Ï¿×$2#é".À96"4ÕËÀ:z&­é²·@!Ë仯@"Á¨¬\?âA{_ò®ß?áL!¬"2Z@«ã	O4@Aý#,?ç…"~°	¿ïB-¡ú?î•TûÚ×R?ä˜Wz:¿ä…"ÿ‰b•¿êî~F¬ãPSRpsr3FGL J1811.3-1927cPSR J1811-1925?ØÅ
ܤ?ÑÈÖ_Ÿ;?ãþûz'®?ÑÈÖ_Ÿ;?íh¡.¥w?Ê­D¥½w´?´ºö"ÔM?Ê­D¥½w´?ã47új?¶³Õ"Ä/«?ٖý'Ä+?¶³Õ"Ä/«?é£Þ4ýô?¹Ü­Øâ?Ép‡ó,/?¹Ü­Øã4FGL J1813.4-1246¿¡Ãã9f6r@Š.ÝcÀ6×1ªœ÷À:O"}Š@öÃì(ˆ@?_[°)ÿ?'D$z¼<d?Ôª±ïÑ´"@<ÜÇÀôQv?úû]ƒé¯?Øhà¿Ô¿Úâ'[â©Ù¿ä²)³W°Á¿èѵ¿¿óö¿î2ò yI¿ïþ Eð¥PSRPSR3FGL J1813.4-1246PSR J1813-1246?pVâJ˜?¬'zì'rž?ïßR;kéÈ?¬'zì'rž?G—­'Ô?Zω¦:ñ†?ïú>Ú"›?Zω¦:ñ†?"ì<ü ™½?‹×b÷¦?ïXžû1?‹×b÷­=PÇð˜=mšYÅþÈF?ïÿÿÿÿ÷=mšYÇ@Ka4FGL J1814.4+3132¿Ú8œN3—8@5²køvŸÀ:LsGyBÀ<&_ċµ«@iº-ã¾@÷òeÊ?ĬÂkIû?àW.ºþn0@±¬Þü+@†Ð.C¿ìw6b'œO?Ԁ÷Áíö"¿á³p:$¾ü¿ãˆáá¿îÞ>s³¿ïòýƒMýºPSRpsrPSR J1814+31?Qxc˜Ý:(?Yé¸Àž¸Š?ï÷CÎ3'c?Yé¸Àž¸Š?'ÈÿT¢…?¢Ò5§´?ïq¸ýZì?¢Ò5§´?›¬&)Ԋ
?‹]6$ûo?ï"žÎ±[¯?‹]6$ûv?†'Qî+k?p¾ŠN|¿{?ï¥ö»¤GS?p¾ŠN|¿{4FGL J1816.5+4510¿êò©i`Ð@8¼`ˆÖÔÀ9O¢ÓÔþÊÀ<Hm'ÓÒ{@e}x£U?ý¤y&\‹?°!ñâî¢?ØOŽÞ§«@$­1ã§Û?û˜'©í?åÞo÷ß ¿ÑUU|´0Ÿ¿ÖXZ_=¿åW¤A=b¿ëße‹u¨¿éRlžä²PSRPSR3FGL J1816.5+4512PSR J1816+4510?[°4K í?VEê!?ïò'óåÚ0?VEê!?r͒.ÎøÃ?|kÙ/z%;?ïÚdÛ¢b?|kÙ/z%;?ˆ"Û>–'?m@N'–°¯?À"§?m@N'–°æ?*+R ՗…?"
	"M×?ïþ]JÝò§?"
	"M×4FGL J1817.1-1742?æòI0çÂ&¿æ¢1ƒ/ÊÉÀ8Xw…À:žé|/üG@侊ê™@^¯ûÛ®?¹¢e^î;Ì?ÚL®ÁI@Åðáy?ùžv*úÕ?ïzÙâ)U¿Þ×q@ŠØ¿ÞƾÀł¿æe}'%¿é™ ºö
´¿ïÿý`éNäPSRPSR3FGL J1817.2-1739PSR J1817-1742?k´Ý¹'IË?hÈ0™Fþ?ïäK"F}·?hÈ0™Fþ?‹ýB—âKØ?–¹‰,l?ï
õ vÑ?–¹‰,l?®|uømßæ?¡‡×½Ö?î8 y"?¡‡×½Ö?N&óŽ9©?9Ì®iÃä?ïøvC~ñ?9Ì®iÃä4FGL J1823.5-3020¿î42ÀŒˆ¤~ÏêÀ8üŽ~³dFÀ;ðåÍNÒÌ@H"Î;G@4²ú"¯u?­‡€sw?ÒãÚzµRÞ@ C­Ò^Ý?îŸ)º_¯?ؽa4"¿ÙØWdÀÉß¿à8lXï¿ßÓ~—µ"Ë¿íÔ§¢òu¿â#ÎÜq…~PSRPSR3FGL J1823.7-3019PSR J1823-3021A?"T+Ü?¾YÐ:̝9?ï]^¡ïø?¾YÐ:̝8?'Y;²?‹U6GÐ?ﷂ˜É7?‹U6GÐ?š¦5V›?"øƒì{§?ï/BÎWÕK?"øƒì{¥?!^‰0ö?SÙÝÎ>?ïþîšlò?SÙÝÎ>4FGL J1824.1+1013?ÊÖ\';¨	@%NÉ:qÀ9»Œƒ"_À<tЌu@Hkԏ@c—>?½ø^öÛi?Ö"›Á,Î@ýKÁŸr!?úT"úP=°¿äª|`"Õm¿Ú_3Â$RE¿Ü8×¢hË¿áîg`¿î*= ÿ:¿ïþÃNžÊPSRPSR3FGL J1824.0+1017PSR J1824+1014?|šØdŋ?tbéd@K?ïÆÊO6té?tbéd@J?à6²slË?˜2¢Fœ'º?ïxþJld™?˜2¢Fœ'º?Œ–8»Œ?ra¥=€Õ?§?ra¥=€à?¢Gµ¡±™?‰4{£Ù[´?îۄ¥äî÷?‰4{£Ù[³4FGL J1824.6-2452?§sÎƉ9ÀfÕ °åÀ81Må"À;6ÕÓËò@ùmqÈoE@=">5ŵ?¬Í`né?Ößf'¥"@$\_|gZ@Ø¢' *?ìå€UÐÂ?Ëoä¿\̵¿ãN'¯rHó¿å*lO´s:¿î™l¸þæ¿×·b|×ÂPSRPSR3FGL J1824.6-2451PSR J1824-2452A?6Ñyø.²?-&Nõs"?ïý%ÐÀú)?-&Nõs"?x@­FòÝÎ?€Íãý">S?ïÏ~¥rD?€Íãý">T?‡[†ò.¯?v-âol§?éä7F?v-âol§}?$º6£åg?ePLâï½?ïþ¾Ô\•Á?ePLâï¾4FGL J1826.1-1256?î¢`_±ZÞ¿ØžžôÀ5°¦#뗓À9:FÖ~&w@Šp8ø,@Ú j™Ò?•4Ú¼P?ەn¼¡0'@@ÉrGE8ï@ùF'¤?ïþ"ÀC§u¿Êzأŗy¿àüDôü–¿¿æ"x'Èœ¼¿íøMïwÀ¿ïÿÿ&¦³PSRPSR3FGL J1826.1-1256PSR J1826-1256?ÑØ÷Ò5ÿ?Ûºê‹õ­T?ç"þå?Ûºê‹õ­U?CEáÞgP?U8aJ
ë¨?ïû.‡ˆf!?U8aJ
ë¨?'YTFғ?†Ò¼óg?ïu5_ÝÉl?†Ò¼óa<×´%í	{B<ÿ)¸
?ïÿÿÿÿÿô<ÿ•·ê,¯4FGL J1827.4-1445¿Ç
󌃿ø<äŒ×êÀ8cã\[J©À;+ÞUõÖ@Y\·Ý@m²¥Ú¼?¿K¸ÿÕ&§?ïÿójÆGx@#ØÛÎÈO@udǪϿâMš¢®R?ï9žÝ%`¿Ê²wa
†í¿ãÝek"£'¿ïùãñ¬€&¿ïþ䬽bÌPSRPSR3FGL J1827.3-1446PSR J1827-1446?sgMÞÀ…•?ªˆ"CJyþ?ïÙ1dB~õ?ªˆ"CJyþ?aǃÜB6¥?mÉcñ"?ïî8|#½É?mÉcñ"?¥ÒxŠäÛ?œ"
ª«	?î¢ØwQ²Q?œ"
ª«	>Âyi$>´щ%ö??ïÿûa¥˜·>´щ%ö?4FGL J1827.6-0849¿íÁ©œeMF?ótx]ï"À8E`؇ëòÀ:¶6eÃ@s¶0(@¼>	P?´A? ¸m€?ǸTÝ¡±@ÿ¿ž ß?óôÃ¿ÒçƒÝD¿?ïðÏ@D"®¿ä¶ÉöX·Q¿ä±F^‰"¿ë:¢hJA¿æ"ÌàîÂÁPSRPSR3FGL J1827.6-0846PSR J1827-0849?€+»þ&k?¢•Vß¼?ïþ¢ Í?¢•Vß¼?|(ÔNiB?‹›;ÍÌ!?ïÇ®Wc,ã?‹›;ÍÌ!?ÇÎp¢d?²@Îë=cç?ê{£×fþ?²@Îë=cæ?gYäßÜç?V$ñ€ë»?ïè¦ø "?V$ñ€ë¼4FGL J1828.4-1059¿½œ¡k;c?£1]<F,À7¯<Kà©#À9½Ñˆô/è@^Ä[@¸•";"+?½¡§Z!‰"?Å¡… eÑ@
2†!î?û§)Æwô¿ÜW'còà¿ÍÇNފd¿è.®è¿è‡B_ ¿ìŠ)º
­h¿â–¹‰$PSRPSRPSR J1828-1101?¸J¢rn#Ö?Ê3ûH™?ìö«±²;…?Ê3ûH™?¢Ö><›Š.?µ;\ªò?îҜ6G^?µ;\ªó?ÍwŽÉgØ?³|
Ã#º?è¾¢M¦
?³|
Ã#º?'Õ †@gí?u¹Çá²o^?ï´«}æþ`?u¹Çá²o^4FGL J1831.5-0935¿ï¡ü"ØôØ?‰"ÏväýŠÀ7íèPïÝÀ9אíùm@Œú#G,å@@E]b×?ïd²Â4˜c?ÔEµV¬µ?ñÕ9eQh}?î%eJ´O¿Ëç‡Ù¿å4µê28¿îx8@8TZ¿ï|ŸB¥ìä¿ï÷8EÁ«1PSRPSRPSR J1831-0952?îºî=!e?À¬`F2¶u?¤Q-î¹Ä?À¬`F2¶u?âSÝ)¶J"?Ùº›#œ; ?ÛXE¬"k¼?Ùº›#œ; ?Ýö˜_‡?´û;{õ}?átú³Ð<?´û;{õ}?lŒJJZ1?/[˜ÏΓ?ïÿ$›­­?/[˜ÏΕ4FGL J1832.4-0847¿âˆqþûr?ÇÔeG'u'À8¡å$w¯À:áî¶+ ˜@ºÑ!Vî@U™Yعj?ÁѨi@5z?å×p>×V>@áµâ¥|&?ÿž5e§?ßî*Àr÷C?ãµ¾=gêu¿Þ5B,Oê¿á¾QtfÚ*¿íáv<?A¿ïÿè«î0PSRPSRPSR J1832-0836?1ÖÿÍ
8_?/åftÍÀ?ïýÅ ^»?/åftÍÀ?zM>%<?ƒOKßIÔ?ïËeƒç·?ƒOKßIÔ?‡É³
š?uŠ@yô_Ì?ï Ù3›×î?uŠ@yô_Ù?ERè¨Ão‹?0È9eA?ïú«EÕÏ%?0È9eA4FGL J1833.0-3840¿àÕÞ"SrÀ*€d©ÍÄÀ:¬îÐ,ӞÀ<£éå‡ó@Z­KR8Ý@5Êd{?ȽÊ{cÏ?à%ô»ÿ/@î­ÕÀ­@{!]æ–?ïã.qÊH?åòØ?ɵ¿Ýè{Vb¿ä Ï§Æ¿î‰›ár¿ïÿԖũÃPSRpsrPSR J1833-3840?½Z{ß¿'¶?¹1bÒì7k?ìT°"
É?¹1bÒì7k?ÊC†²¬ë?̅A.w
?éoS|Å?̅A.w
?ĹÝ=ˆ…2?®qML1V+?êш°Þ³?®qML1V)?Èql"ì7?ª"KWˁ<?éã¤÷Dò8?ª"KWˁ<4FGL J1833.5-1033¿ìW'DØ¿ëù
ãˆÐôÀ79€C‡>MÀ:+-û»Í¡@—Э'Ñ@v¦ã.8"?§IÜÂ?˒Où<—`@ H,nóÓ¢?ñ¹Z¢
¢?ïúGߒ¢/¿ËYý¢W®=¿ä>ÚÑrMû¿ç
U=Ÿæ¿ë
+ãðU¿ç_QŸ/ÐPSRPSR3FGL J1833.5-1033PSR J1833-1034?œ³þ¨²"?Ã~łÏi˜?ï¢`
ºl?Ã~łÏi˜?j±ŽÃ"?ze¨͙?ïåîNqï<?ze¨͙?¥Søœ
°?¦7¾§æ?îªÀ~Ö?V?¦7¾§ç>âÌ
«ô>×&1S
7?ïÿí3õT
>×&1S
74FGL J1836.2+5925?ãŒÛ^%'@9(€QÉ÷À53¡Qô¿ZÀ:}àÖo
@ºMϖ«©?þ$Ã9¦?X±ÊåWb[?Ù=¤¦=@_jcÇOµ@)."?½ÒfÛ)1¿ÀËFý¿Ûοì¹ñ¿åùèÄzô¿î¯Úê¿ïÿülòPSRPSR3FGL J1836.2+5925PSR J1836+5925?f¡2ü…•?`Ez+Þ]¢?ïé^Ízø?`Ez+Þ]¡?E¦cZQ?enÝää·B?ïú–gék?enÝää·B?Ý/)ºæ?"ë\A/±·?‹CY?"ë\A/±»?ð4FGL J1837.8-0604?åBQ–¯Ž?Í2¦ÆRàÀ7èȼœÓáÀ9¬DmŒË@ W\ÆT¡@öÙæÃ1?Áþ‡ÚÕN?Á8SX—›¾@t#¾K)Ê?ÿý`Îvðø¿åÒJO¯j¼¿Ö™5{aö¿à×:yx'â¿èRœðf/	¿è»°DÖɦ¿ë"^~»qÜPSRPSR3FGL J1837.9-0607PSR J1837-0604?ÃLZxVš?̈–Á^õ?ë,é~!êY?̈–Á^õ?­.ช£ä?¾ƒ*Tt?î-ôwUÄ?¾ƒ*Tt?ËÀ?UlÊÝ?Ãß›Çۅ?éð*¤ÍI?Ãß›Çۅ?¿@NgMØÂ?´v¯z«ø?ìö3Dç?´v¯z«ø4FGL J1838.9-0537?Èï6«x=?ÉzH†µˆÀ6é]…UÀ9¤ßI® @ lëT¢C·@÷é¾u5?­%Åask?Õæ͓œ*@'ڎO¹{·?î}Ððóȏ?ïh—c^t*¿Ý¤¯!k4¬¿árÞyzпãORúȉ¿ëÖWûi˜J¿íCèWlÎ_PSRPSR3FGL J1838.9-0537PSR J1838-0537?»êþÔ?Óq?ëØ9?ìÂ½€=?Óq?ëØ9?VGØi;?c~çaaO?ïôñø\Ì?c~çaaO?'»û<†Œ¦?‹=è•ÛÂ?ïj &˛?‹=è•ÛÏ>iMfY>i܎hï?ïÿÿæ벚>i܎hï4FGL J1843.7-1114¿ïót6¶H)ÀW=
§ˆÀ8Œ»*ƒÀ:ꨆœfÓ@³¸ʏ@FKùӖ?²Àßٙå?Ô]+ß×Ár@¼ó…@=rŸ.ÙÝ?ïÿºà¼ô¿ÛUçÞK$l¿ç™aOü¿è®¯?ôÖ¿ïÿûÎBÓ?ïü>>ÿðPSRPSR3FGL J1843.6-1114PSR J1843-1113?ЧSY~V½?ʵf²üY"?ç¬VS@Ô¢?ʵf²üY"?¼•` Vº?É~< ê¯?ìm\Sûõ)?É~< ê¯?ÊÕ{OÆò?²¶hƒ¬é:?éJ¡,x?²¶hƒ¬é9?žmÂZö"*?'™_§§&?ï'í(Nï?'™_§§%4FGL J1844.4-0345¿ëÆTxA&µ¿ÅDÜþÉBÀ7ˍ¶6ˆRÀ:|TŠ›ÏÕ@ùà×Ù@ÌÕeø']?µ¬]–‰î?äï »ç¢@&W?·¥ô@8g'›%¿ïîB_Ëí?ï[Á&¦\ö¿ØÝ>|¿æàzÉʹͿî»ûXÑRn¿ïÿl\I¬òPSRPSR3FGL J1844.3-0344PSR J1844-0346?‰"xkm?¶‡ZOµ"?S—¯?¶‡ZOµ"?V‡h3Sú¶?bßûÆÐ%ò?ïô¼KæV?bßûÆÐ%ò?œui$œóÊ?–ßQkå¹?ïT¶Ûb?–ßQkå¶>ëùÅ¶Þq>âQÊ*Ðٍ?ïÿä:óH>âQÊ*Ðٍ4FGL J1846.3+0919¿ï¢¯º*Ov@jš^»w:À8‹ÛYÀ;¦1Wà@˜–t¸@xs€?£×r࣢?à¸põ5¢@2Ôm?ž{@¤ŠM÷.Ë?Ëìւƒ(¿ÉîNý"õ¿Õà3œd¥¿â¹q:Õ¾ä¿îD žq¿ïÿlÞfþPSRPSR3FGL J1846.3+0919PSR J1846+0919?`ú°ÁB—0?Y¶Ÿö]GF?ïïO>½h?Y¶Ÿö]GF?W'bÝÖ?jöµ3H.G?ïô6±N'?jöµ3H.G?"ħ1Ê\?Œ`|"e¸Ç?ïaÚÆq¯5?Œ`|"e¸Î>s_b8›—>xÖ²Þâk?ïÿÿÙA;Ž>xÖ²Þâk4FGL J1852.2-1309¿èÀiÏU€À"ý>" 
À:#º
RiYÀ<'@ÿ¥@žD 
é?ÿb‰,d?Æõì€Ç:½?à=òÿf}@{ùiãÉ@\u'ŸVG?ïö.Åæ(¾¿»òªÝ¿ÔH$ÜÙ4¿âg$ÒG`¿ïw^3'þ¿ïþº…¢kÐPSRpsrPSR J1852-13?¥âVâŽ0Ô?¥•÷qú-<?î¡Ú'×ó?¥•÷qú-;?ŏ°G|?ÉÊküÐ]?êœî ü€?ÉÊküÐ]?žÛ˜Â
?'lt/¶XÃ?ï	#?§¡ï?'lt/¶XÃ?ÇUƒL?¥ìžKW-?ê<*¾,ù?¥ìžKW-4FGL J1853.3-0005¿¶¨FŽÀH¿Þz5›mYJÀ9 òxXrÀ;"!\q@ "Dû݆ƒ@–ÖZ²Ô?ÐoÜ†©'?çFz7Ԃ¤@Íÿàè@g ÎN¿ïÿõEq#?ïÿÙÔóü¿¼¸j•6|¿ÚÌaÿÏ¿ë3g5™?¿ïûÓ {‹PSRPSR3FGL J1853.2+0006PSR J1853-0004?¹ßäÓ²Ž:?½6y ;hb?ìÄe‰®8?½6y ;hb?™Ú¯¹²R?¦{É_18K?ï1*‡Ú2n?¦{É_18K?ђ¯	î\?³æiôC…Õ?ç6ö({Ò?³æiôC…Ô?«­¦OÃÄ? .h~{¡«?îE/՛Ã? .h~{¡ª4FGL J1855.9-1435?¥¯Â¾ò©ÀS# îøqÀ9ò".E©À;Ѿâ(~¤@€ô2}@3•#SÀ?¿.æâšœ?ÆӘ•±ƒ@®p:û~'?ýQ§Ù"q?ïöÅúJ´Y?薘ȹAÖ¿âê¹çíºƒ¿ÕÜH)¿ìD~‡Å\¿ïÿ*¸:n'PSRPSRPSR J1855-1436?éÒÈé§?Ã"ÜyÛû?È·ï°ÜYb?Ã"ÜyÛû?áâkfCX?ÔD·ï}?ÝÆ;)3yP?ÔD·ï}?æR(tzŸ?µçªuôV-?Ó[¯û
Á?µçªuôV-?Õâ5L·€?¸52ß Nd?ååY¤s??¸52ß Nd4FGL J1857.2+0941¿ÆðE<Öyœ@ñ|ƒ^À9B%ÁZ¨ÃÀ:àãܳʝ@=ø9âû@þ¥2?Ë°›=އà?Òõv¤¢X@÷Eî Ú@½"ñÙÍ?￶Ï4†¿ÜœiÌ2ô¿é3Î~}´a¿êæÿQ"W¿ì4q ԋ޿ïúFsBîPSRpsrPSR J1857+0943?ÚùÄì"?Í0ø»,Ï?âƒô‰ó=?Í0ø»,Ï?ȱf®€Æ?Ë{èW©e?éý¦T_Î?Ë{èW©e?Û}›š'®?µ|=xœÔï?âpA22·(?µ|=xœÔï?¸ÙÊ/<Z? ÇûyÞ?ìäƺt¾? ÇûyÞ4FGL J1857.6+0143¿éü%q÷¿âÓ_XU+«À9ÐQ¼‹6À; B\›âI@ ìÓRwò@'ß­*p?Í@zï_t?ïÿ¤€RuÄ@r²žM]?ÿäP\8åû¿ãú=‰Mq?ë÷u¢™r'¿ÙÓ7º¿åq"ý€Hæ¿ð?ïÌ+òÍ–PSRPSRPSR J1857+0143	?Šæ¦Np¸?µË_…g`?ï"efÇÆ=?µË_…g`?–W j_Ù?¯Ïè!}åï?ïMBü­?¯Ïè!}åñ?µ–4×s¼?§:뼕k°?íM9eñ‰?§:뼕k¯?3èэ}	?*¥´/	ÍÞ?ïý'åÎP_?*¥´/	ÍÝ4FGL J1858.3-2216?àÙ҇€¨&À&ÉE•5†ËÀ96$)ªô5À<.wîN&Õ@÷ýÙµœ@ɪ`':P?²»dš‰X¯?ä:¾ÖêÞ@)¦XĽ4?ú¶ÛʚC?ïî"ã)/¤?Åvpõ‹‡Þ¿ÐYÏêŽ~³¿æØßT¹Á¿î @gNC¿ïþY¢2ÅOPSRPSR3FGL J1858.2-2215PSR J1858-2216?KAly$Ã?Gzí©š›?ïù/¤á¶ù?Gzí©š›?v[º›?ƒ´Q9/Ti?ïÓIËòäŒ?ƒ´Q9/Ti?†®)›W¿	?e¹·ïÕÊ?ï¥GY'¡?e¹·ïÕ£>½{1£õ…>¸hÔ¬-û?ïÿüP™Ë'>¸hÔ¬-û4FGL J1901.4-0126?È]ps3iÀ¥úÐìÀ8©@GDbÀ;Ðzw@ c°(§>@™,d?°6{<6g?Ôz …2`@µGZ1¤¾@ƒG#€Ö?ìÀÂ}h‹…¿Ìo`¥aÏ¿àÛ¸•Ò¿å#'†Wv¿ëò"a¤	à¿ïÿÿ&¦³PSRPSR3FGL J1901.5-0126PSR J1901-0125?s~{Öa3¼?­¹B€€¡—?ïÙS=˜?­¹B€€¡–?•à¥é¡¶?Ÿhm߃?ïPÿºÐ²ñ?Ÿhm߃?†<÷Ք)?w'æêÕÎ.?ï§ ©¯]?w'æêÕÎ1?C‹ìH†?fï»jöô?ïºñÁÐNà?fï»jöõ4FGL J1902.0-5105?ïâÿý+ˆÀ6`Yž×ÇÀ8'hŒ±SËÀ;¯ð†nD@óœR†Šž@1¸YxAZ?¤—XP µ?ÑòñCú€º@(·×<'W†?ÿQK¯€á'?ìô'ßíæοÔíï\C͵¿ãÕ¥ÿ-¿æÌ£FÁ…q¿îß5/7¿ïýG¾Ûr'PSRPSR3FGL J1902.0-5107PSR J1902-5105?z-êG#Ĝ?'ËŒD¡?ïˤ+q¸w?'ËŒD¡?€?¯¢«ßP?…§fÚãw?ï¿AuP"?…§fÚãw?žeŠ:Øí†?"pš?«b?ïÓ®)8•?"pš?«b>íåY‹Ü¯>ëcW&¾?ïÿâ¦t#>ëcW&¿4FGL J1903.4-7053¿æÚ?¯NgÀ:~¦Á HàÀ9øy5v'À<ºø6#@ŠøEÌgø?þ{9wÑ?·>,á_€ï?ã'Èâ\@!$¢v·í?ÿnãMß¿ëj2±‹(¿Å¸À¦MÝ¿ÁîŒe(£¸¿àfN²Š¿í™ÀÀú܀¿ïøÆ+$qPSRPSR3FGL J1903.6-7052PSR J1903-7051?d\°°×?`².µö ?ïë£=OýO?`².µö ?Žv00:Y?"Y=±2ԓ?ï†'??"?"Y=±2ԓ?•º•E€¢Þ?ˆ(-´O!å?ïR+UÓúé?ˆ(-´O!Þ?a|E§1ÍÆ?Q-¤Ó?ïXÎ3?Q-¤Ó4FGL J1904.4-1129?à]´‡[Œ©À $Ï®ÿ\lÀ:ÇnìFå˜À<dÍßòC@}ÂuÛÏI@£°#HÚd?֋Óyq?ãRE|áÒî@~zÄÂ<P@¾ÒEå?åŠ)ýýÇ¿ì&á`'¡°¿Ôöǝ
"¿è€ôËۿïÿþó…õ?ïöÔþIœPSRpsrPSR J1904-11?ïRò'¼Ñ.?˜u 5Ýýs?•¡­ÈeÚ?˜u 5Ýýs?T,?³¬a¶7؛?¥5Z½8?³¬a¶7؛?艖µ!¿?¯óD»÷N?ÍÙ¥+{Ý?¯óD»÷O?ê&'`*
?°ûmÃ.ó	?Çe»²WË?°ûmÃ.ó	4FGL J1906.4+0723¿í²ê\ŠÁ?¬)¹úµÀ7Gg"s—§À9ÝZ±&~@ÔŽþ
2@%¸ m]Ñ?°Â÷Æ´?ҘnáµD@%Ԗ$š@°6ú*O¿ïcÔ?ïø{§@KJ¿å4>vn¿æº¯ßV¿ì£¶ôs®¿ïÿ#+~3PSRPSRPSR J1906+0722?¬Õ‡_ì?Ê3µ|Ù.?î2®Ÿ—Š?Ê3µ|Ù.?Y\ç
Ùú¡?fÿë؅ÏÜ?ïóQŒy?fÿë؅ÏÜ?¡ì=Ž˜k?–P	öD@?îá<'yN?–P	öD=>Îý0&ÕS)>ÌÝ,R¥w?ïÿø@³öK>ÌÝ,R¥w4FGL J1907.9+0602¿éO'X‰\¿ìÔpÄÜ>À5äÜÊpÑúÀ9¾ÕöA:]@€Î(™Ò@Y9W9£?€×@ÕCz?Ó
Žÿä:@?Ÿ‡ð#ê@A‰Km¼œ?ïìu¿I×e¿Ô€ä+Ž#D¿áú@m®YD¿åÒdáÖõ¿ìøb²|¿n¿íãP!U*PSRPSR3FGL J1907.9+0602PSR J1907+0602?FP6]Â8ò?=Íý&õ£-?ïúkòhr?=Íý&õ£-?GÙ¿àïî~?XÛ¯0Ò5Í?ïú	Ä?XÛ¯0Ò5Í?'j›*Ë¡Ë?]Dè緗É?ï¶U"TÑx?]Dè緗å=/©ê¼q°=HfÉ7??ïÿÿÿÿþ=HfÕ=ën4FGL J1908.9+2103¿îåа;®@è^ùŠ›À:7ÉÞÛÃÀ<Ó;{×@ÓÇ­©@±¢|—*T?ÄïL>h?Ü¢)` §@ö=Ÿ@Afl›‰´¿Àôš	¿çù5
¤¿«lи¿¤›¿åLx~–ÞÔ¿êáfµN+¿ïÓ	'Où=PSRPSRPSR J1908+2105?²éØbnÀ?µ@¡ËbsU?í¢Äó²>‡?µ@¡ËbsU?ßI7÷R†}?Ôÿ±t¡V?à[dV¼À?Ôÿ±t¡V?ÄèÓ£]oa?²Ç`×9?êÅË(¤(?²Ç`×9?ßõÒËqU?³¶Q½ûtt?àzšGU?³¶Q½ûtu4FGL J1913.3+0905?ì˜ÖIÙª¿åñ|‰'öÀ8¯YAºµÀ;0Ž=E@d"iS֗@ñÓíR~?À÷ß`"U?á
&"¿?F@¿b€þ˜@³8•¶Š?îœ"_ü?¿çædžJ ¿Ý %ú»r‡¿äÑiêe¿ïÿôÂ_5›?ï÷ŞÛ!úPSRPSR3FGL J1913.0+0910PSR J1913+0904?­] `ÖªŠ?Çö/ûõÑ ?î*%ùò•W?Çö/ûõÑ ?¡ÿ(Ðä§?º#+¤_?îçà
rñ¶?º#+¤_?²áËWX?ª:fô¢ê?í£Æ•?ª:fô¢î?L$ºäa?D°ÏŽ¼a©?ïøöÑxFè?D°ÏŽ¼a©4FGL J1913.3+1019?éÏÑmŒ¿½÷'qøÀ8º(8-m÷À:gþ¬Bê@!¡žJÙB@& }¹i?Â6F¸÷?²n·Ù»s?ù…õB6Ü5@*ívæfQ¿ß`nŸðË°?ïò´BgXª¿×
¼;Ú÷ˆ¿å ø0'æ¿à®2ã'ø¿ç.uÉ°¸šPSRPSR1FGL J1913.7+1007cPSR J1913+1011?ëf»ÂÅ?Á\ŒÙ•r?Âg§Åôî?Á\ŒÙ•r?é˜ýŒ·Ð?ÑøȞr15?ɜÑÍ À?ÑøȞr15?éøJE¨PU?±áë'ðgÚ?ÈÖé^¾©?±áë'ðgÛ?꼊ñ²"¿?°P¢I‰¥2?Å
Ô95í?°P¢I‰¥24FGL J1919.1+2354?ç¦Úð•¡~@å9û¤P­À:µflE£xÀ<Š˜¨ØѾ@ÏÓ)`G@ãŸý`éO?ҀóûØÑ?ïü³åu:?@_–ž<–‰@£º	P¶§¿î«rßñm¿ÝiÚ¤¦½ï?ÞUIž¶™¿ì²ZÆ3¢¿æ¶õ׈¿ïÿѧ' ÖPSRpsrPSR J1919+23?Â~'rbßÚ?ÁöˆKqœ/?ë`[cgH	?ÁöˆKqœ/?±UýÏ
Ðì?Ä"Rëu?íÕ@F¥ã?Ä"Rëu?Ðçê´&?·§ª­±xë?çŒ
ð%öí?·§ª­±xë?¬‡‹?ždÏÌo?î>®ç‡NÏ?ždÏÌo4FGL J1921.1+1930¿ïO¡Lõð@ÃA2Ð7À:YP¦á€¹À;Ù'æ÷ñ@ 
Ž?w4@Ã/M= ?ÑcꠝCó?â©þk«@~Ó½Ö.@̸
Íóé¿à™æõlÿ¿èž÷ýR%½¿ÛõÀ¥Í¿ÞVe9q'¿íM,Ù|Þ¿êÔÁÔiPSRPSR3FGL J1921.6+1934PSR J1921+1929?¸ºÈ©	¥?¿Ð®<_?ìè¦êÞÎ?¿Ð®<_?¾dñŒŸ%T?ÈRúšÜ/º?ì3aÎlV?ÈRúšÜ/º?Ñ-ºS]å??·"kz¾MÀ?çi"ÖQ
`?·"kz¾M¿?Ì`BÑ·T:?´ §iÒû`?èçïK'*ò?´ §iÒû`4FGL J1921.4+0136?ïÕjTÊ<À·rÁ¾{ÑÀ98èÑQ­À;Ù¥J_ @"ãð)ô@÷¨»uŒt?µ™ËÍ]÷?Òù,Ü×ÜË@M;ÞÓ_Ž@×£—'?堟²¸N'¿Þµý½ÛmO¿ßîÝBæ¯w¿ã¡¸LH
¿ë`0âvd¿ïï\ÏõPSRPSR3FGL J1921.2+0136PSR J1921+0137?wÁ\Ïg
?v½½ÏZ?ïÐ}Fa1ó?v½½ÏZ? t£Öñ£‹?§,¸:¸ù?îøµÂåÇ?§,¸:¸ù?¤DkÓ¯å?—möP؉\?Bů?—möP؉^?'cGyþlj?{7ª&<Ê¡?ïlåÄ0?{7ª&<Ê¡4FGL J1925.2+1729¿Ûâð2I2?æ'ÛçlÀ9ah¼O§À;:²<þŽ@(QغÂ@Ût´?Ê]?5Êè?ä"ûmI@9!ßyx@ÕäÎvE¿ÛxH[c}ÿ¿âÄôÉ_¿á5^Pp¿èõPPx¿í‰"Ô7û¿ïÿþó…õPSRPSR3FGL J1925.4+1727PSR J1925+1720?|fq;"†C?÷N[‹y?ïÇ3‰ºò?÷N[‹y?–o@…[Í!?±9€À@?ïL…ûÕ!˜?±9€À@?­•V´B,?šÙH(#Ü?î&®*"»Ý?šÙH(#Ý?g©a"­®æ?Tù'•ëÔ?ïèVž{RQ?Tù'•ëÔ4FGL J1932.2+2221?æ&zÆûh¤?ùYº`úÀ9ÄN`	UÀ;s'È@½S¸cß#@Hæ=·´?Ó=`]¸Ã?ۉQÐ9¿@M}|,¡I@š@Zãü>?îÑÇ]w)'?ïý¶ÿÛíÒ¿â—DŸí˿刘ö«;¿ïܤ`œøÊ¿ïù¿tµÎPSRPSRPSR J1932+2220?Ð܀á[Z?ɸò·Y-ö?瑿|RS?ɸò·Y-ö?¿aã<XËö?Èß=¶Ž
e?ìØtæ?Èß=¶Ž
e?ՎiÙFî?·Ë¶<–÷Ç?å8Ë}"\‰?·Ë¶<–÷È?»5y×ìN?«¤hWïqV?ì™PÅ}6?«¤hWïqV4FGL J1932.3+1916¿ÔœE~š¿?µb©ëJÀ7~ÔÈCÑÀ:Ž•yy@•ŠÀÏ6@¬Ÿ€cg®?¨'¼«ë¬?ÛUߛªd@-ïÓh'1@>—û^ۃ?ɍQâ É¿ÐB3µ¿âé¤ÿ~Oç¿èÛӀE4½¿îf«esø¿è*AA¾¼>PSRPSR3FGL J1932.2+1916PSR J1932+1916?,Ýü¢Õ1? €ÌÄÙ?ð?ïþ2 5Þ²? €ÌÄÙ?ï?Rxäu;Çö?`l«'t?ïöÍÅb?`l«'t?ƒQbݗÐ?^'{¼Õÿ?ﲺt‰£¯?^'{¼ÕÖ>|ÁLroå>|Õ_®$Êþ?ïÿÿÆ}Ág>|Õ_®$Êþ4FGL J1935.2+2029?ì6{F8ú¢?°¼ÿ¿KôÀ8fpȍ£À:~E܃#6@Ú	Òg@±áYKË°?½(Eëf?ØPø€"Ê«@"³Ïà@{έw?Ôy$ä»ÖÛ¿ØH€aå"Y¿å¬:†
˛¿ì!ùOÖοïÿþÐñ¿ëÈ:a$ÞPSRPSR1FGL J1934.9+2031cPSR J1935+2025?Õ.vw£7ª?Ô:L¬üº?åhÄÄ.d+?Ô:L¬üº?˜òN&÷Kj?±/AGaÛÝ?ï8mŽÈE¥?±/AGaÛÞ?ÎêÀÜqPî?¶L~)jð?èEOÈã«Ä?¶L~)jð?|`p"K<?j]ŸZeÑß?ïÇÝ?Ùj?j]ŸZeÑà4FGL J1939.6+2135?âo' ¿ÒÚ
ã]Ý×À8â5~gÀ:Õoê›ë@.|Ì.lO@§ B•¦Æ?¿æ"´4û_?Új{ßI| @°lÊ-¶@Žg£'aï?ï²;†¾Ë'?׈Šþv=¿ã"~aÚ»x¿ç«Œ‹¿îŸ[O7¿ïÿý¡UûŠPSRPSRPSR J1939+2134?O*«•"2?aRc£E%=?ïø85U·?aRc£E%=?€e{'ìú¯?'ê^
ÇG?ï¾j´L?'ê^
ÇG?‰Y<_¢Ê3?|vñP¦É?tÖ?|vñP¦Î?M›­™¿Õ?9DHw(S?ïø™™??9DHw(S4FGL J1946.5-5402¿»@ˆïçAÀ='…¹èÄzÀ9q0ž-}À<§'ÍÍ}Í@-µ"2@5¦à©ùc?°x±'ž‡?âÄ ¾{ü%@(ÐkYnL?ö	¸éžÀ?ìÔ þþ"Z¿Ôÿž[JT¿Ô·ºÁÝZ¿é‰²€ñ,(¿ïÿ«çy÷=¿êO]ë­¹PSRPSR3FGL J1946.4-5403PSR J1946-5403
?T9ľ4Ó[?cï¢û<?ïõã å—?cï¢û<?†F'ô?ŒQUL]øè?溜Æå÷Œ?ŒQUL]øç?'¯6$à2?ˆ,.¨?ïr†NØÿÅ?ˆ,.¨>µ\®—ag>°üL?ïÿýT*+>°üL4FGL J1950.6+2416¿Ãþ`ŽjZ¿ò[vH[¹À9Z`,ÃÀ:Ño™\@ˆªFJ@Á¹Þ³?Êuú	?Ðеd¦GÓ@
¸S 8"¬@øᬭÈ{¿êÓà뽩?ïÿ$m'M¿ç`Jù"–-¿çÛ?áíEh¿ïüäW-
¿èü{±QFDPSRpsrPSR J1950+2414?âwÈJ¸Ìì?Íë]ɪ¸~?ÛojŽf&?Íë]ɪ¸~?ÚxFh?Ó%PW{9?âóÃý\þL?Ó%PW{9?ÓO'~þ?µ2•Âüàß?æsôØ6À?µ2•Âüàà?Åõì1;{g?²ÞiœaÇ?ꂄó±!&?²ÞiœaÇ4FGL J1952.9+3252?î!?Ÿ+]<@"™Iè^À6¨V˾°À:¤NA¬rº@G¾"¤9@a59°€?'	ÉSØ?ÑÏrä¤@<¤Y!…Æ?ü°ô9MS›?ꨏ òSo¿Ð"žry¿áÇggî%ã¿å¢l ºŠ«¿íB XÐ{®¿ì†XVÙ+PSRPSR3FGL J1952.9+3253PSR J1952+3252?R]Œ{î[Z?[óõâ^Ü?ïöÑ9ÂÔ?[óõâ^Ü?G ó0;?]v«èîÆö?ïúûƒ3?]v«èîÆö?ƒÄ@Ùï?l</¶ã?ï°îÿŒ˜D?l</¶Ð=qàáäG¿=ŒY-›"?ïÿÿÿÿÜ>=ŒY/k4FGL J1954.3+2836¿çî˜?»×?×â4½÷ÇÍÀ6òçø¢=­À:{(‹9"†@ODL
D§@‹Ÿ}ß(ð?œC¦·©?Ô¼íÇWæ@4ÉîEÃX°@àp©?ï÷uýÞÄ¿Ì¿¯î¿à²¿-¿åÛibš)¿ìhÄÓTÑ¿ínúSPSRPSR3FGL J1954.2+2836PSR J1954+2836?FÚFþüÊ?C²&º™ññ?ïúIn{€A?C²&º™ññ?G:!p?Wü_
Âhá?ïú1w¿~{?Wü_
Âhá?'ú=w—ºð?cè¿2ý0?ï´
!¡?cè¿2ý_>#x:Sè>0-ÈØ>%Ç?ïÿÿþÆ({>0-ÈØ>%Ê4FGL J1957.6+5033¿ï""hˆø@&	»j¤¹ˆÀ8eŒ«tqÀ;ϽƟŒ"@ýÁ@¸ýé¥K?¨®'zšÇ?威‡ª@5¤A»Œ2©?ý]!ŽpÅ?î݂AŽ?É¿ÌÝÐÀ¢G¿ãµJÐê°¿íP,h=Öû¿îÚG¿ïÿMéDÓPSRPSR3FGL J1957.7+5034PSR J1957+5033?Q´m"`'ý?YdXËo?ï÷%ÉnϾ?YdXËo?h5/{-?•K«Ô?…?ïçÊЄÒq?•K«Ô?…?¢$¦}–É3?—¯Ø
S?îݵ˜&"l?—¯Ø
O>&ÕBò†½>Ö.ôì¸?ïÿÿÿ£dª>Ö.ôì¸4FGL J1958.7+2846¿ïâ6öG>¿ÖÚ
'ºÀ6ùgÉÉãÀ:—"rñ$@üi°ó¨Y@µ€e-?šþËD'?ÙoQ|I|¡@8‡Œ!áÒ?ÿd7È]?ïüÏ^w"œ¿ÄY€ú¼I¿àÁOÁs¿ç]*J¿ì£o÷à¿îBãÈÂýPSRPSR3FGL J1958.6+2845PSR J1958+2846?Nq'ÁÒ!ž?NgÚÛ®g?ïøc›O‹x?NgÚÛ®g?L™Á¡…?]†LqTöS?ïøُ—º_?]†LqTöS?Œ¢U8†go?ƒÌ¨_V'Ý?ïv«æb?ƒÌ¨_V'Ù=¾¯]aù­Ô=ÕÓ³Uü²6?ïÿÿÿü*=ÕÓ³Uü¼Õ4FGL J1959.5+2048¿ì5	¤þ¿ÀÄ{gkÀ8Ú·ÿ¶.%À;Àäù}@´šýqÛ:@›ì't¹æ?¯uÝöjÖ?Ü UàÝ%
@%u"BJ'k@•šw?ïÿíUÙPi¿ºÌZ¡Œ,I¿âTI˜ÐEþ¿çIÁ/à˜¿ï-ž§öT¿ðPSRPSR3FGL J1959.5+2047PSR J1959+2048?…›v߄Kl?®mÇÅÂv?禍$îÒ?®mÇÅÂv?v•>Ù¯:H?ƒǍÉÊò?ïÒՂL¡Œ?ƒǍÉÊò?£ÞYoà'?œov2n˜?îÂiý?œov2n˜?«¢y`?W}ŽÜo1?ïÿj¢ïl5?W}ŽÜo14FGL J2006.2+3102?í^zã%Ä¿á<Âþí±IÀ9?ô³›£_À;p.fDØ@ëÏtœ@¬¬Ñ"Âr?Á¡Èg7r?ÚÁl!'J@×Aü#Ò?Ý#Š'ÇpË¿ïþ2Œã(?ïòX½[jµ¿ßՁ;ÔÂe¿å+ùæ/t¿í"XŽÛP¿ðPSRPSRPSR J2006+3102?Åy»•_ûš?Õ$ñJ=£?ꡑ¨?Õ$ñJ=£?†1^´c?¡ÖÏæpø©?ï§;҇ý.?¡ÖÏæpø©?­¢'âˆ4e?¢
æ8êÅ?î%݁×|º?¢
æ8êÁ?Ë|CIÔL?*D³òê'?ïÿq¤å²?*D³òê'4FGL J2006.4+0147?êd'c1À/ŒgœÇK"À:ŠsùÍÀ<¬é\OŒ/@Š"Yé«U?ÿ4?Žò?ědŸç¼g?Ú·u¢™r'@ª•…7âÅ?ï‹x~™?ïÊ\ô‰?·ºä—ï ¿ÍÂ\ÜNõÜ¿Ú¨ÓÞ¹ß4¿êÓÜ¡@B¿æg€)ÙîPSRPSR3FGL J2006.6+0150PSR J2006+0148?ÃTin£	Ž?Æ`è¹ÈT»?ë*å¤W=?Æ`è¹ÈT»?¾­F²,³â?ÌIB¥Ûté?ì*W)ºi"?ÌIB¥Ûtè?¾w˧ܨ¾?¬¹ZÖ±¢?ì1‹jé?¬¹ZÖ±£?|þü´?y±ˆVB1??y±ˆVB14FGL J2017.4+0602¿²{éw>³ÅÀ0Ÿb0vÀÀ8dÝÐ*OÀ;˜Å~ð¡@Ùtæ[ê?úក‰'\?¤ŽÁ¬æ±?ÚDãÿï9@5­¥¹bŒ½@/j¦¼î?ïÔ°á´»^¿ÁAá_¿ÌëõF";¿Ý¶0©7 ¿ëŠ÷0ÇÉ¿ðPSRPSR3FGL J2017.3+0602PSR J2017+0603?‰[l/8¬'?¨ãÔJ	?OCN?¨ãÔJ	?p«&ý±ß´?~';…-"?ïÞ©²œ@?~';…-"?ŸˆÓÿGm?— "‹#þ#?ïù`Ä?— "‹#þ)>G©ùêå"j>VË̙¢"õ?ïÿÿú">VË̙¢"õ4FGL J2017.7-1612¿ã<]©º/DÀ:4ÕÇGQÎÀ9ÎTæâ!ÉÀ<W^Æ^ô'@ˆ*Û Ð@䲁Çë¼?¸	{>d¿?ÑS•ÿ0LN@»Ÿ'x@mK–¬T\?ïê9>åîݿݒK|U;¿Ø¶<?@ˆ¿â•V©Zý¿íÂû'²ö¿änÒ ÷0ùPSRPSR3FGL J2017.6-1616PSR J2017-1614?–ÝSV—?""g¿Lí?ïIeKGg?""g¿Lí?Ë끨
¡G?Ðì¤péù?é•ýW¯?Ðì¤péù?¬¤U8VEK?žkž7R›?î5º¬z›¬?žkž7R ?Ãêô£e?£ˆ»"ÓÒ?ëBÏW&¼?£ˆ»"ÓÒ4FGL J2017.9+3625?äb1_qÞA?Øç;x| À7`C{ÓÀ:l«,i—@Þ$ªÚ3¾@ªY:-ù8?¦ÐNƒèú¢?á߁ëR@1í_‹Î@¨¹(«?j•ExZ/¿ÚlªMF¿àPhb¿è¹¿èîú‰žyÓ¿ï4ör2M¿é"—VÉ:qPSRPSR3FGL J2017.9+3627PSR J2017+3625?0Ì–H0j?&8ÌJ?ïýæ}í6ü?&8ÌJ?O¢â"?apC9 š?ïø8—~Çw?apC9 š?ƒ»kÚ­#?g.˜­bš@?ï±P•Ks?g.˜­bš]>]±)XÚ>ba'aÞï?ïÿÿñò(>ba'aÞï4FGL J2021.1+3651?ï‹Õ(;ú?»ì˜ïû{À5^Ê÷àÀ9¿-<y-@îý­•O@âXýÈ[?…\¼!6?Ձòžm"×@J^$_ZÙj?ý|$C?ÞÔûD"i\¿Ða1ޟ](¿áLà«üÉ¿æW~6fÄZ¿íZhµËÿ¿îqžBuÆPSRPSR3FGL J2021.1+3651PSR J2021+3651?¡¬9Ÿòô?ÄlÝcpU?îå<fÞ?ÄlÝcpU?Ae‹[álú?XÝR
§?ïû¦)¥?XÝR
§?!¬Z‰â?'©‰B[¬o?yN•Ø?'©‰B[¬m?ð4FGL J2021.5+4026¿îuø#l€@§~¼ž`À4æe×Ë-À9E¼Çœd@̧"W`9@èEc·_}?‰ñЁ&?Ù~†TB@Lôów[0@nÇ­Ô¿Ñ&s1P¿¸{w€Ñ1ò¿áÉ^ƒCÿ¿èU±|æ¿îÔvå9«¿îõ_þmXÉPSRPSR3FGL J2021.5+4026PSR J2021+4026?ݨ\Þg²¾?Î5øxS`?á+ѐÌ&¡?Î5øxS`?Df¤+«u?eé9J=œù?ïúý&Võ?eé9J=œù?ÚBÉÄeØf?´Ë¾žð›?âޛÍÍ?´Ë¾žð›?ð4FGL J2022.3+3840?¼UPª(?î=oâ'JÀ8tPrßÀ:‰ƒùdo@8'l+w@i_?*¸?¾—R£/š?Ú8ªkxõ@©×ý'w>@,Á®
¿Í?îZná_+	¿â}]"ðÅпèrçÉ0`¿ç¹" ]îs¿ïÿë<ú\R?ïü›¦2ÚPSRPSR3FGL J2022.2+3840PSR J2022+3842?©?[Ú?¿µ£¾'w?îlŸw*C?¿µ£¾'x?·¿üÏé
?ÇT¹wªL|?íˆfÝ?ÇT¹wªL|?ÎÛ¶®òN?µmC/µ?èIyCm?µmC/µ?g¥K8¨™?[}ÎÁ;?ïèZ´ÇüW?[}ÎÁ;4FGL J2028.3+3331¿ÜÞÒdÀ¤‡3eˆÀ7™ìløÀ;7ý˜F³@ļ YÒ@'ågÎE?¢1R»í4)?䪘Å^C'@8c^t)ž@úúr!…Œ¿è0SðBÛ?ÓÆìM›"F¿ÔôÃ@±öÞ¿çâP¢Yܕ¿î9Pƒ¦N¿ïÿþÞ÷PSRPSR3FGL J2028.3+3332PSR J2028+3332??¼Ð×k?BŸô·šáŠ?ïüeå?BŸô·šáŠ?Rzòèþ?e&èkDQÐ?ïöÂó‹þ?e&èkDQÐ?""lû3£û?hú«‰Õ÷?ï¯vL1p?hú«‰Õý=Å«õ.ߍ=ÖIÞþÃM{?ïÿÿÿú•:=ÖIÞþÃZÅ4FGL J2030.0+3641?çò¸á®u°¿÷ ²BÀ7ìºç£À;EWøåZ@ÖâVÌÀc@Mø±W%?­Fk\?ãÛ'8S-¤@1-û¹@ÂC*8ä¿ïsÎ>º?ïþñ­VåÀ¿Ò@묋å¿å)µ/ê©¿íñ™ O–@¿ïÿý`éNäPSRPSR3FGL J2030.0+3642PSR J2030+3641?j†‡ÇB?qo¶S?ïåðyx8½?qo¶S?W-M%
?g5¦×*.\?ïôqiYm{?g5¦×*.\?–(šú'6?•ÄÄMª?ïN»(.ÆQ?•ÄÄM¦>gŒfö´Î>kªøÅy9Ø?ïÿÿèsì˜>kªøÅy9Ö4FGL J2030.9+4416?é1>æ/€@%z
XÀ7ßÉÇ^ÏÀ;(öýø¾Ã@Vv&LðÊ@Y ¡`7?ª'ýÀ'%?å-‡ÂÁ@0¨…<ƒE?û#H÷ë‰{¿Õ!ΜZ¿¿Õ{½ZéÛ{¿Ûúd_¦¿êŒY?¿ïùºá辿ïqÊG·N¶PSRPSR3FGL J2030.8+4416PSR J2030+4415?CY¯Ž*»?@òBôٚY?ïû)¹"v?@òBôٚY?W¬}Ç	;l?yÒIhˆÎ?ïô)Á{c?yÒIhˆÎ?‰âžè¢lÈ?sÚ7•?ï˜u"]vN?sÚ7ž>Cá_ñà8>F›|eD«?ïÿÿû=Ǩ>F›|eD«4FGL J2032.2+4127?¾SòÞb?ðbá& %9À6ªŽÊ2¾™À:U»¹@ßuÚ!Ê?ÿ· ÈÍcÌ?žYÊC'?ØÄ6Ûß9a@7ÎáXu@7M­ÝÉI?èµólsÆ¡?££ä¡)ÛÇ¿ÕP<ÙO<¿àR©»OÌÇ¿ë†=Á×{R¿íIš³uòPSRPSR3FGL J2032.2+4126PSR J2032+4127?unøñ÷ôM?wþY`Àµ[?ïÕ"?wþY`Àµ[?DmCÔ T?Vÿ¤ãß?ïúä¯
þØ?Vÿ¤ãÝ?¢;ò­Á9?—áì?îÜ@Õ#ìo?—áì>S·rj;>Ü\–¨í?ïÿÿÿ²±#>Ü\–¨ý4FGL J2035.0+3632?×BðØ4¼ÄÀ»K›	bÀ9 ¨,"	À;Ý©Çå@'L
QÍ?þ°ð˜ƒïä?¹§µ\˜²?ê€ÖõD»@(WšÏú@ˆA¿ïÀ‡—ů?ïÿ胸›?¶Øíþ†êQ¿ÙÒ¾éµ:à¿í™pŽR>¿ïî$ïßvPSRpsr3FGL J2035.0+3634PSR J2034+3632?p²1Äu_?nyyKRN?ïޛýœw?nyyKRM?atmD'F?m†L¿«LË?ïî‹û'»m?m†L¿«LÊ?²N:£Ø´?¤o/¾0??í¼¶8«"é?¤o/¾0?>áú&êá¸>ÖÎ셽|Z?ïÿîÙ÷>ÖÎ셽|Z4FGL J2039.4-3616?ïóûuÃw¥ÀBEò×sÀ:`
ôGÀ<œ£äv6¾@­ùÄ|œ3@Ží¥,u?ÀX[
è'N?Ù©íœ@(R. ý@–ÖÇL…?À×½ìŠ,¿ãˆÄvW˿ڟ[O7¿èŸ5_ˆPÇ¿ïþ£ßm¹A¿ï§匷3PSRPSR3FGL J2038.8-3613PSR J2039-3616?ç­…Aøî?È»m³Ñál?Ñð¤õ|%?È»m³Ñál?éhðù
Ê?ÍúèÕÇ?Ê\<ÈñØ?ÍúèÕÇ?׸<ôTJ"?¼.Š'н?ä#á…ÕÚð?¼.Š'л?欱\F‰Y?µg}¿mk?Ò¦GríN?µg}¿mk4FGL J2039.5-5617¿Ù9ªé=ÀB'ÁDŽPÀ8êÀ<Èe^ÿj@rŸÚ¦T?ÿ©D1ˆ8?©Ólà9Lc?ÎSíèÑ:E@#_'`4@6Öd¦à¿ØE2¤—ú]¿ÞÏ|_LØ¿Ýhã«5£¿âfB
f‹¿ííC/)¹7¿ïÿùëñPSRPSR3FGL J2039.6-5618PSR J2039-5617?ÀLƧ™¼?ºÞ@Ï
þ¦?ëìÎV'?ºÞ@Ï
þ¦?'œÝ^Ãd'?'¿˜yÍË?ïs	äÞ?'¿˜yÍË?ÆB«ÈÇDÚ?³û-õÖB?êoU
Î.É?³û-õÖC?•É{,#ë¸?"&âµµ~¤?ïQ´&žà¤?"&âµµ~¤4FGL J2042.2+0245?қ¦ï°ª†À7	üȽÀ9Ù©?ÿÊPÀ<QÙŽuy@ðªÏ÷Ð@x½ì_9K?¾­odfÜÙ?ä"_¾+Ÿ@@ »'-ºMn@¥P<³?ïÿÿ^ðP`¿×QN¼¦Žõ¿áš'ç°ë¿ìúE`²Ge¿ïþú¡Ç:'¿ê–­ÁnʹPSRPSR3FGL J2042.1+0247PSR J2042+0246?‹4+Ïy?ŒýXÂS?ï"/Pö?ŒýXÂS?†vÑeÂu"?Œ¦O!Hvž?ï¦$ºhö*?Œ¦O!Hvž?­²"¸Æc? EÎúZ"?î$ÖÄ~"™? EÎúZ"?<TåÓ[ÙÑ?*£ ž¾¬?ïüucE""?*£ ž¾«4FGL J2043.3+1711?ãvòÃñª‡À.¢(D€cÀ8H…'òQÀ;½·ý1ïf@f­ZÁ—?ýÿ´€¥¬Í?¢sz ,›??Ó<ëƒFF
@0©:÷LÓ@Ú>›ò{?ïÿؒӬ»¿Ó³ÚøßzN¿Ù Ú@'ãI¿âŸ>HÀc¿ëò¬MÑD¿ïÿÿ)@k*PSRPSR3FGL J2043.2+1711PSR J2043+1711?–Í.÷Nž²?"+"?ïI–ˆE‹?"+"?r¨äÂÕ>¥?}eõÄ^'A?ïÚ®6zUƒ?}eõÄ^'A?›´gühJ+?"úî÷B]?ï"\À½¯?"úî÷B[>¾3
‹Ÿ+9>Â*‹+Ç?ïÿü9ž®Œ>Â*‹+Ç4FGL J2043.7+2741?°A©ì™´öÀ"Jeà.©aÀ9sZôB\œÀ<%ê°¢¦@õ'¦¸'@+e˜U?¶'«hÎös?áëaŠ@ ö²(ܘ@ÆÞ	àÿ¿§˜»"Ujk¿Ðg°Ql¿ái¬}Ãû¿ì¬#ßÙ¿ïÔ÷©i^¿ïÕ@¿ð©PSRPSR3FGL J2043.8+2741PSR J2043+2740?®m"ŠF<?¶ÁµhŠç¬?î'·_{œ?¶ÁµhŠç¬?¤¡Qî›?¾ººyú;*?êîq?¾ººyú;*?Í;DÊu??¶÷CåC	«?è±.þb±?¶÷CåC	«?"x×zï¶?y»mô*\?ïd?¡D(ƒ?y»mô*\4FGL J2045.9-6835?éÇñ*¤ËÀA»>ÄaÀ:âØK%À<ö¥Nفç@ßé"ÃÏM?ü<cþ­©?Ë×î©ksÁ?èô¨H‰Î@uh¿ÜúA@"…£Ãi!?­t²ÄL¿àÞç+ž¿Àøÿ%:¿ãz›#¿îR£`—ÅY¿ïêÈ@ +šPSRpsr3FGL J2045.6-6838PSR J2045-68?°E¾c¯ïC?Âú­óÿr?í÷H3Š?Âú­óÿr?²ô ú®Ù?Á¼	"KÕ?í¡{àª/Å?Á¼	"KÔ?Àv"®øCþ?¦ù.Ô|?ëâ[Aîÿ?¦ù.Ô{?¶šÏ¤ºU?¥šÓ›~?í=L¦h¶?¥šÓ›~4FGL J2047.3+1051?ì¹"Ž›‹À3º­æW¸NÀ:K¼£n/À<8öí1Ç"@Tö.šó?û4+'»?Á†}]"ñ?ØθêÑÆ@£'üÇf[@¹ù$¹	¿îü¶¿š4I?½_e@KŸ'¿ÖEìuæ¿Û
b¿ù¿ëLóc9‹<¿å€Þý{ì5PSRPSR3FGL J2047.1+1054PSR J2047+1053?çûÙþ
p?ņÿ´Ø?ÐLåÓ ?ņÿ´Ø?ïÝWŠ ˆ?ßuó´å?qT:ò¯»ý?ßuó´å?Ó?4'²÷à?¹?Y–ÖU?æ`e¾¦"?¹?Y–ÖU?î¹\"`?˜¡NKçÖâ?¯Dj7¿ùú?˜¡NKçÖà4FGL J2051.0-0826?­½Š[J À>cC,¥zÀ:š~dž;ïÀ<¿,Áÿê1@›™¡ýj@o	A=?Ä©h?ä¬(²¦°Ù@Ñ'o°'?ü÷WØYý¿ïÿøþÙå9?ïÿ¼]éÀ#¿ÊöˆÝߙ®¿áaÝøï¿ïÿÏ"èbU?ïõw`‰­"PSRPSR3FGL J2051.3-0828PSR J2051-0827?µ<{Ø)+?·Ÿ…î?íXp"úÝ;?·Ÿ…ï?Ã5ˆ¯'a"?ÎÊàA0ù%?ë2Ôg›?ÎÊàA0ù&?¿=,ւŽÙ?©½½qõ?ìZe/®%?©½½qö?¬ÉÅÑŸ?Å"‡$èÈ?î6óc¢ã¥?Å"‡$èÉ4FGL J2052.7+1218¿ë·€æÖÂÀ3ýµc#»ÇÀ9äÂa8ÿüÀ<(2áԛÎ@>"«n@8Ÿƒ¾f?½–^%Ð;?ÃB'_ŽZ÷@ûšþôg@à?¸o?ﱿàÖ'¿án'xbè-¿âÝ6;ü/'¿æÓ\.§¿è0dxO¿ïíh]â^YPSRPSR3FGL J2052.7+1217PSR J2052+1218?ïʈ,#?ŸŸ"Lf?¼?Ÿ&¼Nú{‡?ŸŸ"Lf?¼?ïp4,‡ä?¡E#œ\˜?'ü¹zoo?¡E#œ\™?íNÌAQc}?¥`".€
p?µ‰õtä?¥`".€
p?ê	ؖ/¹î?¥ßu?>?Ç؝§AJ?¥ßu?=4FGL J2055.8+2540¿‡ÐöD¤K¸À)
7.jwÀ7ªÃvõØÀ;¨ÿ°NçÅ@KüŽ0"Ø?ýpä8ú'?ž:öËù¾?âËt8Ùe@Al?Ä;.@ñœs)˜?ߓ~AÏXB¿«,F¯çº¿ÜÉ¥%	ó¿ê "àwN–¿ï z"Ԙ¿ïÿ atd+PSRPSR3FGL J2055.8+2539PSR J2055+2539?MÇÈƼ
?B2>èV—?ïøŽ
ÎPû?B2>èV—?aeé(º?qݛïk'?ïîšð×E?qݛïk'?…Jý=KäÐ?p^v'õXÁ?ïªÔ
Ðn?p^v'õXÓ=+z3‹*óù=Iܑ(¬?ïÿÿÿÿþH=IçSŸ?4FGL J2111.4+4606?îÛÊÊ¿÷Dº)\ÜÀ7Ä 
a'ÒÀ;Zƒ®Ò@iÚקqI@#.£yè?ž¨e—çñI?а.[ˆ@,Q¾ôœõo@qÁcb%?ïÿ–¹‰$¿Í}÷<7ç¿àø¦Ú'Q¿ã@5z5PD¿ì¹Fk¿î<@".þñPSRPSR3FGL J2111.4+4605PSR J2111+4606?|j¥±Æ£?y¿äim ?ïÇ*µÞœr?y¿äim ?aI¬ý?pU¯tÄ÷Ò?ïîè¶Sê?pU¯tÄ÷Ò?—;;ìN1k?4"4î?ïF& Žv?4"4î>¾ªØ+¬ù>¿¹|\!?ïÿü*°û>¿¹|\!4FGL J2115.1+5449?æfùÑè×@{>—ÔÀ9«Ã½Y'CÀ<H:vôS$@ AjT‡–¸@S%A(Ï?ÀÞjÄoF?éyvCS;ç@ Yªu[Í@5euû…¿ä'pÀ²b=¿ßò([¾Âž¿j‹éÐ
;e¿Ü=eü‰(¿ìòª¬çT8¿ïÿÖ"î9PSRPSR3FGL J2114.9+5448PSR J2115+5448?:±ÑØ?@Ï;ȹ3>?ïü½¿©ÅÍ?@Ï;ȹ3??{9¦ØTý? DÈ֝Lˆ?ïɌ²OVÿ? DÈ֝L‰?žTsvÝ(¥?•±Uï…Ì?ï
\dI¹?•±Uï…Ê?.øJ¼Ö¥4?·ó™²?ïþ{T2•?·ó™²4FGL J2124.7-3358¿±•2qÁ÷ÀF¸øa¦
EÀ7ú=ú	FÀ;Óc7ݼß@꓇0á?ùp0dKÙó?¡¥€­oÊ?àÿ‰kV@=÷Ú+Z!@)‹ê"n?ì0`†R•?Ĭ	É,"B¿ÐÆÚ¯ä^º¿ä>÷âz3"¿ï"NB_Ì¿ä±ÈcäPSRPSR3FGL J2124.7-3358PSR J2124-3358?‡~5¢@1.?¹%8V9Ù?ï¢)vÿ<?¹%8V9Ù?€ò—o¶Ìá?¾4Ð ¦?ï¼5¢A$Í?¾4Ð ¦?ªlOu[¬£?§
Ÿî§Ä?îY;ªE5?§
Ÿî§Á="dOò'À=²vz_:)Î?ïÿÿÿÿ\Þ=²vz_:˜4FGL J2129.8-0428?Î*¯ú2yÀBz弇Û+À9»†ýX†À<WêpKÂ@PV¤&c?üûtëdg‰?¸+ƒ–%F?ÝN-?SR
@ 4)ˆ;£@)nÑnòý?ïøï]€¿²ê†qÏt¿×Â??°ï÷¿å•yyh¢¿ë·ù1~'¿ðPSRPSR3FGL J2129.6-0427PSR J2129-0429?†'˜Äñä?¦ü4Ý"º?ï¥õœì;›?¦ü4Ý"¹?Ž*Þ*pA?Œ‹3Œ3©?ï‡W܇V>?Œ‹3Œ3¨?•k¸oE[?Ž'È£"Œ³?ïT§B<…Ö?Ž'È£"Œ±?}c$GTÖ>?kÃÜ8£r#?ïÅ9·qVR?kÃÜ8£r#4FGL J2140.0+4716¿¢‹y}°EÀÌ~É3»À8X«m×sðÀ;ÈY±L=Æ@3xÁ1ãþ@}`ݐi?¨Gq¿Ç?ä¹V}»Â@2fz–¼?ûÃrƒU4¿ÐË+!–Ó—¿À¯HW‡¦R¿à}·³àm¿ëSž­ÕÁ¿ïÿr;†¾Ì¿ïÿ÷Âé±PSRPSR3FGL J2140.0+4715PSR J2139+4716?\ó¼¼Ì?]~FŒâi?ïñ†!ü¡÷?]~FŒâi?z³ºÚþÅI?¬g½:Žs*?ïʘŠJw?¬g½:Žs*?Œ¨J""òÂ?x•tÊùÂ?ï^Õ¯t5?x•tÊùÂ#>2xïcç>6o{g,*r?ïÿÿý°ïÃ>6o{g,*s4FGL J2205.5+6016¿ïö]<si@
è<v©À:zD& }¹À;¼š*¹@"5ÜP£@¾mþ
?Þ
üÂÞ·[?ïýÖZHŒ@¹'m-*@äBtä¿ïÿÞ°ô)?ïÿó5bB¿ÞEÿÉú5¿â…¾'bE¿éû/¶¦ñ¿ëù¦_$ӟPSRPSRPSR J2205+6012?Ý+iŠg0!?ÍþiëĬ?ájK:Ìgð?ÍþiëĬ?Û3ÒMá?Õ¡ŒŠ.?âýæÙ?Õ¡ŒŠ-?㡒*Ì"?¶ÊÉۈ?ؼ۪xç½?¶ÊÉۉ?ÒÃ͂ò5?¾5¹Ÿ­l
?æž>·†å?¾5¹Ÿ­l
4FGL J2208.1+4058¿­øíŠÕÀ(/ëkôDáÀ:ÚøßzNÀ;÷։1@éÏç3€`@=r6~AN?Í&¢+8'ï?èÜsÔ
2î@
ç-@™Á1¹?èQpjÌ&µ¿ØTfB
g¿ì|º–¿åù`ß=虿8ˆÊ¿ïÿ5À+SÁPSRPSRPSR J2208+4056?è‰M;ñÙÈ?Ì>
ƾv?ÍÚË8˜Þ?Ì>
ƾu?Úé:*Uv?Ô@ș:tH?â‹bêÕDÿ?Ô@ș:tH?â
Åí=0?¶`Š†'¾?ÚÅêt%…Ÿ?¶`Š†'¿?¹¡"67,O?¢XTÐój?ìË͙9v?¢XTÐój4FGL J2214.6+3000?ܨ&g‡ŽÀ5¬9-Œ*À8)"UUÀ;Þ\Nµo¹@û—OgqS?úð.½§?£U$'ìG?ßmrÿÑÜ×@9ÔfõŸ@§]žk»?Ó˜ÂÚÄ¿»ã3–…h	¿Ö\²3¿äʵ€í ¿ïÿéYËMq¿ðPSRPSR3FGL J2214.6+3000PSR J2214+3000?•zÔdö?²·zG5Î?ïT)_äØN?²·zG5Î?q•Ï7‡"†?}¿†R?ïÜÔañº?}¿†R?"̳ATÓ?×ûhck?ïYše÷
[?×ûhcm>·weØàˆ>`ÝÜa™Œ?ïÿÿÿ"$>`ÝÜa™µ4FGL J2215.6+5135?éN·¤íéDÀ­6 ¥ýUÀ8̎eˆðÕÀ;þršQO~@kÛÎóB­@—‡B_ ?¦}	bvº?ÒÅ-¼PÓ­@#%">5ŵ@Wå¢0Áê¿·,£Þ'N_¿Ö§]CýÜ¿Ü-l…]¿ãý/5w±¿ìg ÉN=¿ëò¥Z'"PSRPSR3FGL J2215.6+5134PSR J2215+5135?\¡ÁèÍIK?Ožƒ'Kß1?ïñ¯™Z?Ožƒ'Kß1?€ÀHpV?ˆ‰‡·ú
?ï¿ÌÿŽÞ>?ˆ‰‡·ú
?ŽjZºð/?‰^µ½*~(?ï‡ÂV•??‰^µ½*~&?\ʧ†Œ*?N9'`½ë?ïñšþ¬<º?N9'`½ë4FGL J2229.0+6114?ïÉÊC©@–Ü»WYƒÀ6þ"ÅõÀ:}E$Í>ã@ë
ò[ý'@h
"'r5?‰¥§Cü.9?ËçÂÇeYÌ@A[5Ÿôým?ÿ2̾_ Í¿¢T(÷(¿Øj¾[›¿âÓÄ"ïï¿åXåó€¿ì;E»Ëó‰¿îá['—PSRPSR3FGL J2229.0+6114PSR J2229+6114?uÌ^qQð°?ˆK–¯?ïÔgC\?ˆK–¯?Pž´Óý×?h¦
#t	E?ï÷°ð%–?h¦
#t	E?±Š¢t?1?¥rç7pz?íΫ±xù?¥rç7py=.'Ñ"= šü´wü?ïÿÿÿÿÿ´= šÿÁ"4FGL J2234.7+0943?ä§s	GÀD8ªà"À9WÿÚ@SÀ<*øÞ£@ 2×àÔ@-»à~í?²üPý+?Ú=ë]†˜á@!@åæyF=@
£Àäâ?ÛÛ°•^¡v?'9jYåúp¿ÚîädC '¿ãf0€ÑK¸¿ëùd€LP¿ïÿò^VÍlPSRPSR3FGL J2234.8+0945PSR J2234+0944?¤ýÓ*×?¢W⏏U6?î¾ "ÍS?¢W⏏U6?¦'Uâ Gí?½¶Ç@Ç?î—Ú¡Õûƒ?½¶Ç@Ç?·» ໝ*?°è²¸Ú6?í›ãèŒ\?°è²¸Ú6? .¥$g›?‰¶Ã˱?îý­¹†G?‰¶Ã˱4FGL J2238.5+5903?ï0/	C,?Þm:åÚÀ7tKAFò-À:×¥œàv@ßùߪu	@øB0üø? mXaÚªJ?Ó£{X)b@1¶®::Žq@=ØïÅË&¿ÈçV¦Tèæ¿ÕZºá'׉¿âø¾eUð¿ç‹Ýž¬(¿íÏ@ãȒ¿ïÿ÷œ"/¥PSRPSR3FGL J2238.4+5903PSR J2238+5903?[rU_?XËí¢,ä?ïòFøÕP2?XËí¢,ä?Pèbo×¼p?`½@2ËÊ?ï÷‹ÎÈ"?`½@2ËÊ?'†r˜¨ò?Z¤
ø2‹Ü?ïµç'5]?Z¤
ø2‹¡>nÜðŽ5™š>r
ʸÞdI?ïÿÿá#r>r
ʸÞdI4FGL J2240.6+5833?ïiB‹Æ¿¹äÖg3À9eNÀWs"À;'ÊÇ9@¢	ç4'@Yr|õ%?¼*Ë/¾´†?ԞG=×&@³q*Ç?ó÷Œo?Ñ6þï´®?ë·3ÞSÝοÝá'ÑÖ÷É¿åÀʀAXæ¿ì䥜[d¿ïÿ¼ä!}(PSRPSR3FGL J2240.9+5831PSR J2240+5832?d3†Ê'tD?gñêíè(?ïëÌy5}Œ?gñêíè(?ˆ²ü«á—?¡k­E{?ï4
P{©?¡k­E|?˜qdˆÞb²?›øÐËØ?ï<tÛ¹ë?›øÐËÔ?ZXŠ©(;?J&¿MjŽ?ïòÓº«kã?J&¿MjŽ4FGL J2241.7-5236¿ÑP…ÚðÀKw' ÿT	À8e½²}–.À;…ê&yçM@'´§«€@Ôœ¸2?¥W]bW?à¥Ç¥EŸG@6üa'?þr܎`ÖZ¿°±×þÚ,?£PAá̹,¿ØĤà¹)¿äƒÇ4ÝW_¿ïnàR»Ž·¿ïÿ»ËǔPSRPSR3FGL J2241.6-5237PSR J2241-5236?CŒ;sÖÀZ?6ÅQT˜?ïûñ#
Q?6ÅQT˜?9Sœ~~?†MØ_'­<?ï»±Ž	?†MØ_'­<?…ÿ鍱?x¢¨ð91ù?ï¨[ýÉ<?x¢¨ð92>¾˜ŸpGÜ>5dM³?ïÿÿÿz:>5dMÅ4FGL J2256.8-1024¿ìlÉlÐRÀM#b¶®}VÀ9¥[n¼À<EÉGÝ@Ž%·õz@?ÿbîᵒ?µ¿'Ò€?ÔGÁSœà@éö©?)@k • ãû¿ÒEI€|'"¿Ó¶z¢Þg¿à*‰
ÖØ¿åEcKÿ²Ó¿ïÿ/àîAè¿ëw´!ZBÂPSRPSR3FGL J2256.7-1022PSR J2256-1024?ÄüÏ2¿?¿{bsZŠ?êÀÌ3|Ð ?¿{bsZŠ?ÏN¦´Gg?Ӟpï%g?è,VRî?&?Ӟpï%g?º)¯¥\Ü?«8né‹ø'?ìºßªTd?«8né‹ø'?Ô¨Ü,i'?º
£ï'?å«ðéËl?º
£ï'4FGL J2302.7+4443¿îÌÅNŠÄÀ+ü"«%³À7ý#!m8À;ŸDÔE@§ó3üÝ?úæé¸?Ÿ7‰.<~a?ڔšCã…@9AÅ3?öŠ¸³:T?ÒCÛí㿦ašNË?.¿Ó$"ô÷ŽA¿áÓ{½™Á¿íFñVI¿ïÿ°"—©ÕPSRPSR3FGL J2302.7+4443PSR J2302+4442?e‹//mÒ?\¨÷»U{?ïêýtÐГ?\¨÷»Uz?nmó?~€X?~(5vâ<'?ïá'À~?~(5vâ<'?"ub?"ê¸?l]Æðú1?ï®*w¬V?l]Æðú]=ÐáÙl¶[=ép~ÔïË?ïÿÿÿ÷y=ép~Ôú4FGL J2310.0-0555?êËßAœÀLó5*"8	À9ñº
RiYÀ<ƒ6ª¶øO@bsN×(›?û_틉5ž?¾rø-}½?ãáKŒ]@!#{ñèæ@›ûcŽß?ïöý»'"?ÒýŽ`«fv¿ÓfF…öN¦¿ç<ù jn3¿í×ÆZÂÄ5¿ïÿøÞ£ŽæPSRPSR3FGL J2310.1-0557PSR J2310-0555?dÑIÍ,|?ƒs€ò‡÷?ïºlºØËO?ƒs€ò‡÷?˜Ëöý×ïD?­Ë¢è`îU?ï9 H@†?­Ë¢è`îU? ‹‡[õ?"‰nÐD?î÷GŠGá?"‰nÐE?Œš‡P‡Z³?0ÕªÎ8?â½â•?0ÕªÎ84FGL J2317.3+1433¿ï½Èj/ÀE;^Ès¬À;•'àÙìÀ=$)Ùî@¾CdÞØ@'#[NÛ/?؈•zѐ?ïÿ–ل@£ÃÙß@4ÛÐË´õ¿ïÑ	ro‰%?ïüٍ©Ì¿ÔóÉ[(Dÿì¾YÂi¢¿Ð×ͱÏ…¿ïÿM½øôsPSRPSRPSR J2317+1439?æ`j=òÊ?ÊC—ж?Ó?Á+"l?ÊC—ж?é
EˆS?Ò9ÑGã$?ËÊ뗹޸?Ò9ÑGã$?â­Í¶QÆ?¸AØ»½©/?Ú¤d"\sö?¸AØ»½©/?Ú9Þ¨"¹
?Å^ÀÂm?â㫽£|?Å^ÀÂm4FGL J2339.6-0533?î<âm"Ò¼ÀO<Øý\·'À8Bj4Q@À;Ítj5(@à,Ä.B´?úê°¢¥²?£ÓցVÂ?ҝ)[™ñ@0í·'êy@é\‹{õ?ëVáŽ$ñ¿ÒÅ}Î¿Ö.ºJi¿á^n€[˜¿ìÂåÃ=Ø¿íˆdüPSRPSR3FGL J2339.6-0533PSR J2339-0533?yDÆfOU¡?sKYûT32?ïÍvs3aT?sKYûT32?‹D
Eþ?ªè¬¿º$?ï'ï"ÇÖè?ªè¬¿º$?–¸ýˆþ?"¨i«æþt?ïK'8#¹?"¨i«æþy>ÍX!+¹ë…>ÓöîðÀË?ïÿø©÷µ>ÓöîðÀË4FGL J0002.1+6721c?؎âº@Â[T‹À9Ð'Ai
À;2ɪ@o£c@ëˆÊ>}?Ê©>þž?ÖmŽcZ˜R@¦÷ µí@S³Ü:ÿ?Ø3ºâ¿}Y¿æ­ݨ<J¿âžâ^.‰€¿éB"ßοïÿþ½à ¿?é§fN³OTHERunk1RXS J000209.4+672503)?ÅÙNwI™…?ž]'b‰?ꉬb-™Ÿ?ž]'b‰?Ñšöºi\?џ߭"à(?ç}2"¢ËR?џ߭"à(?ÉUpˆ‰­?±M¨k×?é¹j£Ýݔ?±M¨kØ?ÐD6D£è?¶ÉÛÁâV˜?çÝðäÝ®?¶ÉÛÁâV˜4FGL J0002.7+7220?ï‡sR{ÐR@#¨–»˜ÇãÀ:hã1" À;}¹?QN§@e	Àóû@H_ÐJ/Ï?Ð<ÌÄ¿78?²[¿ïCÅ'?çFùž¼ï	@HF6p)‰?î–ÿöÅě¿ÖOæ<Štä¿å	Ñ:×B¿ä"è™¿ï'Æ0ÑY$?âãA&
OTHERsppSNR G119.5+10.2?ïÞ!üá*?xêýÕ»*û?pïøk9?xêýÕ»*ú?ïmþxêí1?²ûw¿ïœ?'@0â¢Yã?²ûw¿ïœ?í½]ND´¤?¡ë[uŠ®·?²ÚZâ?¡ë[uŠ®·?ï'dp°Å?gÂv±/?‹¦Ø£ÓÎÒ?gÂv±/4FGL J0024.0-7204¿Ù€°œÌÀFr¾ß¤@À8Yø©ÊiÀ;òkón!F@y§¯†ì?ûäû,[¨?£g¿j?Öìþ{E›–@4¸Œ£è?ú"Ï»¼Ë?ހeëí#"¿¯kR3~‡š¿Úàr%uZ¿ä.b"óè¿íè«ð´2¢¿ë©;}"OTHERglc3FGL J0023.9-7203NGC 104?]Æ2g½D?R9Ýô>,?ïñôfÌ!?R9Ýô>,?€r¨]Ð¥¬?…Œ»ï;x?ï¾5^ˆ½i?…Œ»ï;w?"Êí/à\?nÕuF¦?ï¬ÔKC"?nÕuF»>_Ž]yÔýô>k¦˜ŠõB?ïÿÿð8ÑC>k¦˜ŠõC4FGL J0025.3+6408?è4ˆrÅÆ?ö¿ã°> ÍÀ9Yº !ÞwÀ;'µ‹g§¯@ "CÆS`û@dŠ=Ü¡?³á_èE?ˆ´¼¾?sç?ÖH¿aÕ2?÷>ó/âò?ïÿjCj¸Û¿Ê˜†t"è¿Ü•qaEg¿åÏ2ؚ`i¿á"?Žò¿çàÌÞë]\OTHERsnr3FGL J0025.7+6404Tycho?ï§WÉ~™`?ð"æ–=g?†*
 Y§ú?ð"æ–=f?êzn;²W?Ð+†¼Ì53?ÆEû6¢?Ð+†¼Ì53?î}OLÀKX?š|˜?DŒÄ?¨+3ûJ?š|˜?DŒÄ?æ¸nÄe…?¶yN]7¶©?ҏ"w5Æö?¶yN]7¶©4FGL J0043.2+4114¿Ôõeè}×À5š¬§"W`À;
"ßþعÀ<fI¿f²½@-¤€¨[ÿ@0\"U?Õ'،°?æPràÈ,@M7 '½´?öؖVîú¿ÞDD}ˆkõ¿¬¸€‡qú¿×Ç
â@Ò¿îž/á5¿ïÿ¼þùoÃ?≲€ñ,(OTHERgal3FGL J0042.5+4117M 31?ëF—u?Æ&*¸q*?Ãã÷îå¢,?Æ&*¸q*?àì­9ªo'?ÖÒh,¿Pz?Þ&¥Œ« Þ?ÖÒh,¿Pz?Ú÷;@ӏ?º²%=î×C?âðb_–8?º²%=î×C?͎;•g›Á?µ{K,µ*?èœq¦?µ{K,µ*4FGL J0047.3+6943¿ïõûÃ+@iìb"IÏÀ:ç¬è*÷%À<TBcQÞð@!BcMØ%?ÿ*'5Îîæ?Ê=£N¤(?¤0bp-?Þь"Þ ²?üë¯Ï;¿ïÿª¥Z—ü?ïø;`(^Ä¿åÑ3~²†¿Û"½'Æf¿Øþìɹ¿ãMòfºI=OTHERunk1RXS J004724.5+694222?ïým"4l?3€…®~?4—ûf\£m?3€…®~‡?ïä摡?ÏûÒä?kãn^á?ÏûÒå?ïè)TŒ©å?m¨ž(Û:ö?gÖ«sV‹?m¨ž(Û:û?ïs"+ã¾?'¿"S\Ӛ?'ÏzƒˆT?'¿"S\Ӛ4FGL J0047.5-2517¿ït.V^ÊYÀUþ	þ†ƒ<À9¸×ï?¾\À<'~b¯@¿jë@,^,Ü?²zãáfaß?».Ï¡=|ã@	þÂé<@RÙâ)U?í8ÙÀ¦"ê¿Í]ª?¯…¿áÁVw¿ãú¯É†Ç/¿æ´EL:k6¿áágßjrOTHERsbg3FGL J0047.5-2516NGC 253?ï´&M¡O"?ƒyš…Êë5?'öl—¬7s?ƒyš…Êë5?îú`=»+Ñ?»˜5F\Ï? Yü$MB÷?»˜5F\Ï?î0®ýG×? 1䈘>j?¬þu+'? 1䈘>j?îô¾üÛ?‹¾¬3? ´?þ2O?‹¾¬34FGL J0058.0-7245e?éNÐà@J•ÀF/Ne¾ ºÀ8f֕£jÔÀ;~ÚÉÒ+@<›=އà@üÅ2¤—ú?¥ª	ÜÖ7ã?·e~"é×@ò–pm@Pބ°(|?ïZ˜1º/¿Ü°žBö ¿ã1Í7U×£¿ãdâ¢÷ç-¿æí¾Ña‡¿ïÿDN
ª
OTHERGAL3FGL J0059.0-7242eSMC?ë=Æ¥éĀ?»(¹àF?ÃåhXî?»(¹àF?¼¬èJj3?Çù½}q¤þ?ì}Jbö²º?Çù½}q¤þ?êçd!Ç?¯pÖôõij?DZøboxå?¯pÖôõik?ÐòäNßf?´BÔâåŽ?ç†ÿØL?´BÔâåŽ4FGL J0059.7-7210?ìäHS¤YÀFwè¢ìÀ;$¡¯ À<pƒåÓ.@;uÒêóÿ@¯0¿»lR?Õ~aDh¶?ëc݊Š2@4	t@¼•Dj¿îÍ=ø:?åüO{пç£ôÑΔM¿íç	Ÿ&¿ïüÖë3À!?ã'‰|$TOTHERsfrNGC 346?è²á~@lÙ?Èt <r?Í4zþLž?Èt <q?çúÉ¢?Óñžz"XB?ÑÅÍî
l½?Óñžz"XB?ᘙ%&å?»(Ȕò/$?ÜÎ͵³Ô5?»(Ȕò/%?༁Ó'ÿ?Àõ62©?އüXú?Àõ62©4FGL J0102.9-7051?ïýb¸Ì~ÀG¡ô±îÀ;@X|™À<Ȟƒ
f@ñà¬Óˆ(?ú¹_ÒÎn?ÙjCä'?éäNÿA"@uPÊï$@š6ù¼D?îð0Ä#¿íÝ.yÖ?Õç[ƒßH%¿æÐt!:k¿êÿsFT¿ï5?†'ÍOTHERglcNGC 362?ïö(ÕpÕ?bRG5Ë
m?S®UÃU³?bRG5Ë
o?ïíÖÁÑÏ´?…ó¥ÖOã?b)>.0Kq?…ó¥ÖOã?î`Ä3æá?šò2‰h€h?©ó¼È'ï?šò2‰h€g?ï_üÄR?Š#P¥?"|ÇuÌ?Š#P¥~4FGL J0138.6+6821¿©ËnÂë6´@ƒÅ¢6 MÀ9Á%q©ˆÀ;‡tߥíe@7fÛ¬8®@ú}ªOÊC?¿æùß)›°?³u67õdÆ?ó®K½m´9?íý°ðMZ?ïý'w>$ÿ¿ãþyC¿ë-Z˜¿çM	h^Ž+¿ä©,I4&x¿å¹^Æ^ô'OTHERunk87GB 013451.9+680621?I6©t?¢eäÝ
—?‰­²U¢þ?¢eäÝ
—?嵙ç"c–?ÔQ?À^'ß?ԔÌ1»8Ô?ÔQ?À^'ß?í'¬J6Ý?¡BåZÔlÜ?³ïڝ®I?¡BåZÔlÛ?Ӗ3"åf?´Qdâ` ?æ4æ6
xL?´Qdâ` 4FGL J0212.1+5321¿ï"ØÐ;D‡À…‰ïØjÀ8ÚÓC"LÀ<|ûÔ!U@Å0L£òŽ?ýàBæ.¢?«ØB÷¡aº?ؚÐÑ>K•@)0"»?ö­—}_§¿ÙÎ"Ë+b¿µèüoq¿Ü¨b_EµÂ¿åj	=ìIÀ¿îeÖS^Kæ¿ïõŠ@`B`OTHERbin3FGL J0212.1+53201SXPS J021210.6+532136?dígŠ?hõs˜=ˆf?ïë˜üuì?hõs˜=ˆe?tI*†
Úµ?€àڏl'‹?ï×mªóêJ?€àڏl'‹?"§ænù?i©Ì!]TÂ?ï­aÀfG‰?i©Ì!]TÑ>鑹kAZá>ål?%ÊçÂ?ïÿænF"¾>ål?%ÊçÂ4FGL J0221.4+6241e?ÜòDŒ?ü°?ù—?·¥ôÀ8PÃí*:fÀ:ˆ ¼8*@ò§|Ü@@dß}©y?¹S;€""í?×|CG}m@d@y?ô†@Æï" ¿ã¸Û~@w¿¿¹Ó/<ƒ"ô¿áÃGb• Ž¿é@>aÔ¿í)Ãèø|~¿é+
oÆOTHERSNR3FGL J0224.0+6235HB 3?RSK*µ ?X	ђã ??ïö·ÖZj¦?X	ђã >?ù'%þÊZ?Ÿ€`±t ?ï¸÷h×?Ÿ€`±t ?…yT÷M ?oæYMy\?益¬"Ê?oæYMyP?EXpÝM*?2'&Ü
¼?ïú©ãûˆ¬?2'&Ü
¼4FGL J0222.4+6156e?¹Bä9y×?íõ,ÒÆáÑÀ6ã'[·¶»À:;`z"@½…TÖ@v¥xÊí?š±Œ¼ú?л0J@0}?À	oë@âFHä S?À›ïà"?¿Ó5"FK=ì¿ä°>Œ,ɍ¿è*¹¢"ª$¿ì틉5žG¿è=¦S¼?·OTHERsnr3FGL J0223.6+6204W 3?Fõ$ÇÀÀ?_â.ì™?ïúB¶ÎÐ?_â.ì™?PA=ï|jƒ?`°ÛdÔ&É?ï÷ßaAË?`°ÛdÔ&É?"}…¤·äš?ˆÞ«]L8–?ïdÒÚ@Û?ˆÞ«]L8š>vÛØöéy>zÕµ¦~ïO?ïÿÿÒHNy>zÕµ¦~ïO4FGL J0240.5+6113¿ê$â¡ö‹?ñfþÂ^§À5zÚÿ•wÀ:èâ­â@P'ԅRæ@0Ҁjôk?~>n-bÂK?ÂôæÇIÖ
@=[oâæê…@Vo"w¤¿ÀNÿYfú¿Þ‹É'—½¿äæMà^¿æŸŒAœƒ¿ë¨{Ÿ2µµ¿è,¿0|uOTHERHMB3FGL J0240.5+6113LSI +61 303?âp-a=?ÊO9±µ_ò?Û¥=Æý…?ÊO9±µ_ò?tËQv?­
y{*-Ã?ïÖiãýû]?­
y{*-Ã?æ­å!"é…?¶8¦šç²Ž?Ò¤5¼Ø,÷?¶8¦šç²Ž>¤ uÊÀƒ>("¨lo?ïÿÿÿbÚý>("¨lq4FGL J0242.6-0000¿è™»'†TÀI÷%€ÃÿÀ9ÁN_¤À<Iʳ!@æG¤€@'šCㄟ?±ï¥ö,? : ×ùÒ?ë~‰¬¼Œ@Iύ¿âuác\ƪ¿ÝT»ÊàŽ¿çPÝ»1š¿æ?2Ȫ(¿ÒKÃãD2Š¿ïÿŝƒ‰OTHERsbg3FGL J0242.7-0001NGC 1068?ïûk—É?A‰÷†¶A&?C'Q£è۝?A‰÷†¶A.?ïýâð—ä{?K¤gښöí?0è{@Ü#ß?K¤gښöé?ïÓÄ>mõ?xi qV°¿?vwàɬ?xi qV°¸?ï÷£¾áø?EfJW/<?QÖ¸'<;?EfJW/<4FGL J0328.6+5330?êÞį°iÀÀ­È"#^À9øxG9zuÀ;£ãŸw)@ùqcÅwC@öVhÂa9?ÈBÎFIm?Öiü¾, @€_&×@
$àŠó?ï­Ä~Ÿ˜6¿¦=žàÅ¿åkB£é~´¿æ–akTâ°¿ïý®KØE§¿íþyzϪOTHERunkNVSS J032847+532859	?Ê}2œÂ¸ó?Ã!ìŽ#|?é`³XÏQÃ?Ã!ìŽ#|?ÛÈ,+cñÞ?Óð¨Ñq°?âéêN?Óð¨Ñq°?ϼ…¥å°d?µºDʲ?èޖ†"ç?µºDʲ?Ã8;<bw?£á‹¸f¸?ë1ñ0ç{â?£á‹¸f¸4FGL J0359.7+4445¿ëkÚéQÀšÀ0=µm5À:P "ˆÞ`À;æÝî]@M@H¯å`l|@È!å-ã?»ú# Ä¿©Œסçò?ïùÓ`dĦ?þ"EÇ	"¿êf"¿˜?¿'X¡p—\¿ìÏÀÒÆӿטh û£$¿ë^>¿ƒc!?áÏÐÝӅNOTHERunk1RXS J040006.3+444512?îiN1äF?¨fÎâÔ?©nûữ?¨fÎâÔ?ïƍgB7T?—@ºT4é?|¹L^äU™?—@ºT4é?í-,ç
àí?¤#öÝ9u;?¶–˜Çø›?¤#öÝ9u;?ïZ«Y^îû?"ö0Êêï]?"ª"Ô" ¢?"ö0Êêï\4FGL J0402.5+5402¿ßfš6gÓ?ðƒ
%ó¯À:ÔüøÀ;ñ4ØNá@"7ÑÌ?ÿx¹º¡Q?ÊÜ@Þ¡,?‹`Ŭ`àY?¾Ó¯êéÃ@›ØÚ¢"?ÔµŒßvó|?î<xVRó?›PÇåÿ›#¿æ—œ~ÑAQ¿Û0cu^P¿Õ×Ýašy¾OTHERunkTXS 0358+539?ïòZ‰1Èã?jÑ6'4,?[Jíœn9ì?jÑ6'4,?ï')Ýh?²‹ú"³>?‹uˆ¥û;™?²‹ú"³>?ïvA2¼Õ?Žñ'¡°Ö?'7Ù¨oÅ\?Žñ'¡°Ú?ḯDî"?njWùÆ?y?]õˆ¶±?njWùÅ4FGL J0427.2+5533e?ë5º€àõ@P;£D=GÀ7éè¢ì(³À:Ìûƒ¶@"JjꯋÉ?ùV~AN~é?§þÅdÆ?´Æ´"×j¶@Á`@Q{Œ=e'¿ïÿòɶ—×?ïþÀ//˜t?ÔHk^rÒ¿Æ­ò2ql¿Ôàœbvª¿Õ¥µLOTHERSNR3FGL J0425.8+5600SNR G150.3+04.5?ï+'ô'Us? ùÚ]c|Í?š›mÕQ¢? ùÚ]c|Í?ß?5ؕ?Ú^qJ(8?à`|eµ~?Ú^qJ(8?ꃼ¡¢m?±ƒè¥ÚÜ?Åñ
yw¦P?±ƒè¥ÚÜ?Ô#iÛà™?ÁðK<ÄX·?åîK@³?ÁðK<ÄX·4FGL J0427.8-6704¿ìµ¹×LÛÄÀCFž<–‰DÀ9{"ÆäÀ<XÚ")@·«N!÷@þxük 
?¬e BÖr?"~­Úï$f?äsÂÚۃI@ïÒ#ù¯Y¿äÂB…5´¿Þ
÷9‡á¿æêL¼ƒ©¿äy'EÖ¤¿ãà>>T#™¿ê˜iñŽOTHERLMB3FGL J0427.9-67041SXPS J042749.2-670434?ï굇?K–?bZ§á÷Üe?eJxÀ´jo?bZ§á÷Üe?ïó¥`øœ?~¢,ü]?Xµ?úÈF?~¢,ü]?ï"âH<Fœ?‰ãúð&}Ø?ŽÇmðîY?‰ãúð&}Ö?ïÁM' ì?qÛ¡àÙº{?Yl|oŠR?qÛ¡àÙºx4FGL J0452.9+5117?Ý»•0|¹?@…‹W"<À9Ò¨Žÿâ¤À;m0•Ê@@ŹE˜›@¸PXÝç§?ÇZSÑä?Ö¥¯Q'Ã@é.Àë­@ݜ²üÂ?ÎK™›òå:¿ÔUäswÇ¿ç-v% Jù¿ëð\>D^T¿ìí8™¤¿ïßøÞ£ŽæOTHERsppSNR G156.2+05.7?áÚåA£¤ª?ÇÑÕEf4?ÜJ5|¸¶¬?ÇÑÕEf4?ä+Y N¨?ÑoŸÆ͗?ש×M¿b¯?ÑoŸÆ͗?äµÔê¾?³ìZê¿
"?֕ÈV+ԅ?³ìZê¿
#?ç‡%?ê]F?ªÙñ†zaœ?Ðñµ€+Ev?ªÙñ†zaœ4FGL J0500.3+4639e¿ï¦,ZéÅF@‡?i¢[À8:œÄÞÂÀ:ÊØ£š¤@ïCÿ‰8@:–¹ëH¹?±®+L	?Å2évј@k˽Ù@ÒFö^—¿£—ìÆ<e¿Ôä±z¶Õj¿æ×2ƒ2¥¿ä€µ¿ë%F Û¿éøDŸÂ'­OTHERSNR2FGL J0503.2+4643HB 9?²Ôæ×~³d?´'¯Ÿ»,?í¥c%)"?´'¯Ÿ»,?§n¯‡V-V?¼"9hùÔÅ?+?¼"9hùÔÅ?×þí_Z…?· ^Þ%÷?ä‰PR½u?· ^Þ%÷?Á£çs˜ì?¡~°šjƒ?ë—?F#Å?¡~°šjƒ4FGL J0517.9+5030¿Õ*K¹zö@NÏ~Wô´À;í$[)À<uŽÀøƒ4@×̃%äÁ?úÒ
#opÑ?ærÙ;p—?ç©8¨½ùË@;šÅ都?þGÙbÝDê¿ïüD=é?ïþašNË?¿ãÇ}Øró¿Ñ}Nñݨ¿ìÄÝëAú¿º_Êø®OTHERsppSNR G159.6+07.3?î¸é rPº?¢
æÅó%?¤qmøÚôa?¢
æÅó&?é"=G…çq?Ï·'žì?ɳ
áèb;?Ï·'žì?í!3KœŽ?£ýAaÈÛ?¶öe£ø?£ýAaÈÛ?ç²ÛÌâT?µo3š¥›?КHf;WÎ?µo3š¥œ4FGL J0519.9-6845e¿ïñ«UÑÀ@±'¡ ÏÀ6îñ<îØÀ:\pšœÎØ@C¡lv˹@Z5þ¿Ž ?˜Óy—ϼ?ż°µj¬@,H2ËŸ@5ëq…¿À²ŒÙÔG¿ÒÄË¡~•\¿âóó¢y'¿äªúêíID¿êWºÁÝZ¿ÎH"•sOTHERGAL3FGL J0526.6-6825eLMC?|'9-y?"GË¥ëþû?ïÇþۍ¤å?"GË¥ëþü?'P6g•ê¦?†D»¦öiB?ﶿ&a¨U?†D»¦öiB?Ï%_$íè/?µÒ7
Е)?è6¨6ąõ?µÒ7
Е*>âkdB ¯>à}•šÇl?ïÿ픛½^>à}•šÇl4FGL J0521.2+1637?Þ¥©©å®,À&©O‡À:–E"I$À<!]×MY@ëÉa2tò?ø~Ûrýœ?؃b¯É?ïNH,¿{«?ÿú"5¬Š7@ŒÕ»Þ¾?êfÆ"Ž A¿èðaՈ¿Õ@˜Á­^ó¿àåQÉ oâ¿é*‹"ÞQ¿â9¾'‡.]OTHERcss3C 138?ïÛ{¥×(~?v}n–Þ?rB-kÁ)?v}n–Þ	?ïüKÄ·?c:DØ?=§ߺEÒ?c:DÙ?í"Ø•äš0?£d½gA?³Ù;PÛ.?£d½gA?ïé#º%·?_'²)\?fÜEÚHo~?_'²)\4FGL J0523.3-2527¿ÚÛKÃøÀ=Ô2‡;ÉÀ9$éºC]MÀ<4x'@>^çÁð¦?ú[™hò1á?±
Á$"8?ÛE"~°	@)
fðÏáT?÷¡º¢¨¶î¿Í÷Pƒûø‰?£Drö—¡r¿ÔB©Þ5Tö¿âo9©nù³¿í隁öæ¿ïÿó5bBOTHERbin3FGL J0523.3-2528CRTS J052316.9-252737?mHï>­¨?eM‹ôœQ?ïâ·ÁRX?eM‹ôœR?ƒ±"‹é×?ˆGÖ%©Á?ï³ý;uÐY?ˆGÖ%©Á?›ôýx4b=?™ÕQ4~âM?ï X>\î?™ÕQ4~âM?YÈ.¨?֓k1h?ïÿ®›¼ß°?֓k1g4FGL J0524.4-2413?çø‹ ²Æ.À=3ÚÄç%À:©VI¸±À<:Ȇìî«@R`¤.É@`Eºõ4?Àuf3¦¿´ì×?}ªŒ?íB–%œr@¯p¢)‹¿Õ|qÀŒ¢¿èÒ±þ•FÏ¿äö©Àd¿êáÏ=jn´¿Üz¡Ü´ "¿ïÿ⾦™\OTHERglcNGC 1904?ïýòv5#?3hc[?0lOÖVì?3hc5?ïù`•'#?gùØ~EM?J}ª÷sš?gùØ~EO?ïÈÚï'Yb?|êÙtl?{'ˆ6ÓO?|êÙtl?ïñ±¿öÇ?M([Æ|l?\œ€üsé?M([Æ|l4FGL J0524.7+4824¿Ú£èP"|@6D#EfÀ;š%FáeáÀ=G'u¦@ úèóžó¡?ý}ÒÉfÿ?ÛD^ÞÜ?ï¦jÍÔ3É@s''%Î@Ÿµ§ís¿éÆl`{jÚ¿ïÿâ¾÷!?ïþFŒ¬KM¿}87Sÿ0¢¿ì=˨	žå¿ïÿúâôOTHERsppSNR G159.6+07.3?ïˆ:GR
?"GÂů*~?ñ®+}p?"GÂů*?î'·s?ÃbØ£²¤?¯çԎÎÕ?ÃbØ£²¤?ì ÇL
¥y?«ËQ²?¾ùşªÔ;?«ËQ²?éÞÝ–e?º"¯úçšÌ?Ëø"‹ý¦j?º"¯úçšË4FGL J0524.8-6938¿è_†³]nÐÀ@f>lLYuÀ:¯wOµóÀ<>¼(@ P&'º'.@#\ƪsÜ?Ƌ«Dfâ7¿q;ÞPÎg?»7…RdѼ@sÎáÏé7?îF7òµ•¿çM|5Om¿ëøýbô´¿×̤½äý¿Î±ZÖeQé¿ãòEÍiª¿OTHERsnr3FGL J0524.5-6937LMC SNR N 132D?ïô':²?U©qeˆï?Wèý±Ššõ?U©qeˆó?ïý¦ÁÀÄ®?U*!uQ(?2Éñùږy?U*!uQ'?ïÐ1ýèÕ?{JþdÇ~¢?wç•uö?{JþdÇ~ ?ïñažÓÉ?N 1Õ1*w?]=øÂXo¬?N 1Õ1*u4FGL J0526.7+4254¿î_õßþ,@<"Þ ²'À9¶5•
BßÀ;‰Ì·ÔD@r§qsŠ¼@'»0Ã?À=̀{æU?ÎÎ81ʨ@	Š]ò#žk?ûR-ÝZ¿ã>|b&:ҿфîê3¿çžfB)EI¿æ'¿BJ¨E¿ïþ&@Üi"¿ïÿ‡ÕK÷OOTHERsnr3FGL J0526.0+4253SNR G166.0+04.3?Ý%Œ;é©y?ͅËtœ?ám9â+E?ͅËtœ?ÇÞðv§?ËÿÏ=º¶?êCâ}Ö9?ËÿÏ=º¶?Öè8a?ºÄ?¶9;8ø¿¬?ä‹ãÏ`"ž?¶9;8ø¿¬?֋÷Ûʎ?µTcñO?亸þ?µTcñO4FGL J0528.3+1817?Žÿږ{CÀ"zd×ñÀ;
mzVÞ3À<bً÷ðg@""¦ö¤b?ù£l-Î?ÒêsÜp®¿?Ó<'`
ª@Å@Ìxé÷@Ug"xû¿¿ïÿúŒ"¸'¿ïϯ l²?ïÿõMõVY?_³nØ¿ÇÔñžé9À¿é÷ƒŸ‡DWOTHERunk3FGL J0528.3+18151RXS J052829.6+181657?ïú¾D@C¨?A'}60?Eîþñ\É?A'}6(?ïú1ôú'?dC=š%¼?G§8,õð?dC=š%»?ïšöèÛþQ?†P¶i—¶V?‰BEÉkÉ?†P¶i—¶V?ïªÍ\N4'?zQ´Œÿ ?…L¨ìrß?zQ´Œÿ"4FGL J0533.5+1449¿ß­"àÕÀ#•ÿ'+¾ËÀ:æí1Ç"iÀ<8|É:s@!M³ûo¢z?ø\'þ!?Ôèî Y'Â?Ùâwä"?þ ©¨ÛUý@_~ptZ¿çĀ}hák¿ìÃÏ,ù]O¿î—àÓ¿Û?èÙ¿y}¿æ©³ÊG¿ÐWÍÜÂ8IOTHERunk1RXS J053336.0+145115?ï÷üvã?Q–
Îöþó?Pûï:ˆ?Q–
Îöþì?ïø(Éx`¤?Œ?ø§J©D?O\Ú}q-?Œ?ø§J©C?ïY¯7§?ÕøéŒÔ?"Ê\`?ÕøéŒÓ?ïèìãxª?doÁ·VéT?g€‡VJ?doÁ·VéP4FGL J0534.5+2201s¿æDùQic;À 6m
JÀ6"UõÕړÀ8{•É*€Ý@e
'àÃ@
Ÿ²$ªÚ4?Ð^beOæ?åLïg+ˆD?÷±ÇÞP'Ï@ î'š!¿ãq9"Ÿ"•¿í¦È •¡½¿ï·Á½ob¿ê tοêÑ¢ßé_*¿ï
²¢\·OTHERPWN3FGL J0534.5+2201sCrab Nebula?ìÍ­¦ÂlÑ?ÒiwÊÈ÷?¹''Éì™y?ÒiwÊÈ÷?ïýÈxî?R3Ítç/8?1¿§|8'f?R3Ítç/2?èóð?±T—aû?ϳàó0??±T—aú?ïÿ{v®P?	› h?á"Tl-Ã?	› ¦4FGL J0535.2-6736?їޒñÜ{À@óGÀ9[‹]–´À;«qóbbÌ@<°®;Ž@ÅÊz5˜?µ	5'?ÈŸ‰ɺ@d:æ…Û?ý˜ä«㣿©òÕÊø6]¿ç$²1@ì¿æ¥Õ|ž·¿ëP™àç6¿ìC‡¿&›ö¿ï^²"&›uOTHERHMBLMC P3?ۈl8°F`?Ëyxëø?â;Éã§ÜÐ?Ëyxëø?Õ$?Ji?Ó,WÁšza?åvíàZúL?Ó,WÁšza?àÓ·gDI¶?¸ƒu_Ë/Ñ?ÞX'1wl"?¸ƒu_Ë/Ñ?È|ÌØ7??«/Þ§aâk?éû ÌÉò0?«/Þ§aâk4FGL J0537.8-6909¿ïõ!ÈwAÀ?¾)Çy¦µÀ8ÿ[zz¢À;b8¦@!&±ú8•É@Dº"»äG?®!ý"L}~¿œÝÑ_Œ?òˆêõ¬À?þk,kÃÈl¿ïü,k˜ÕN?ïF2nè¿ÛU^–cY¿â/Ljp|¿åðª!§µ¿È÷gjW¿OTHERpwn0FGL J0538.4-6856N 157B?ïÍs'Þ3?xs‹JŠ«Ë?y@F7æ?xs‹JŠ«Í?í֑má?Å'uxÏ?±Kt—Wò?Å'uxÐ?îH£À#á÷? …–?«uÃýÁà‹? …–?éC©È?»610á?Ëêóå[ˆá?»610á4FGL J0540.3+2756e¿ØúMóæ¿÷ÿ@wÏDÀ7˜€dÀ:nÔw»ù@@ƒw3@$Ñ~uY?©f\^rT?¿úBPÝh&@•èO	R?þ`4:Å"ß¿ä7Ö ²Q¿Ò¯&ÿHJ¿ÞÐÏ%l¡¿âí±^\Vÿæ²Ô~«¿å¬Xž&ÇOTHERSNR3FGL J0540.3+2756eSim 147?֋菫Zè?У]ŠµÝ?亸*R‹?У]ŠµÝ?®ÉŒ ô@É?½T–AG?îg5ð»ô?½T–AG?䎶vë?·ALÿ(-[?×Ìâ")Ë?·ALÿ(-[?³ó$m
?–ÈKÅ2í?íž!›r_?–ÈKÅ2í4FGL J0608.6+1149¿íhtۋ€ÀEà.©`·À:5.¬À;´¦Hԅ(@s¿®+L	@M»$-ܲ?Á™UQF¿›'ý\ÑV
?Ú³Z€)0%@eZwÅ´¿ßWú'ص8¿á˜f~9@é¿ê˜!"¥>¿×mÁðzÒ¿å'U¢ÉÄ¿ÛöUDz±™OTHERunkNVSS J060835+114942?ïöVÕ|]›?TdÒJ ?SRUDʪ?TdÒJ?ïþ'éöð?N†˜Ñ²ê²?&ßÑ`'È?N†˜Ñ²ê±?ïpÎK<»h?÷˜ì]ñ?'æ6˜h'Û?÷˜ì]ð?ïôÖçe‰¸?Gˆw}"‹?VR14ìw?Gˆw}"›4FGL J0608.8+2034c?ÉJ…ð—,Â?֒*߈'À9Û©ßaûÀ:ɛëƒq9@™ðX˜—@"‡vf?Æ~ÿyó6?ÆûBÁp£+@0¦ždÚu@@®pì&¿ïÃvõ׈?ïÊÁ$"8¿èË[þ®qB¿åµ¦	êd¿ê°Ì†Uï÷¿ïÿÿ&¦³OTHERunk2FGL J0608.3+2037NVSS J060900+203746$?Ï<aS|ƒ?Ê–í¸Œÿ*?è0ç« ûß?Ê–í¸Œÿ*?ªº)DTì?¹W…y;Ð?îT]kº¿Ò?¹W…y;Ð?ÖIõ[Ÿ^?·:lAÚº†?äÛ7…R0R?·:lAÚº†?Ƕ Ë ??¶RTSçÔL?êWÍÿ°?¶RTSçÔL4FGL J0617.2+2234e?ë>éÆþBE@DÚ`3FÀ5†õ)iÀ9ƒ~mÄ(¹@ —r،I@ýo¿«|?‹¼ê	Q@?À>¯þŠßí@6ú;šàÁ@$&žü?îxˆr)é¿ÐPF~êkÄ¿á_eÁ$øÞ¿áÅÞ,ñ{¿æ*Þ)£¿åWǂ
0ÛOTHERSNR3FGL J0617.2+2234eIC 443?°ŽÍô'Ú?º¯pòœƒà?íî&A{¾?º¯pòœƒà?W´åžb?ƒŠïβtæ?ïôw¥0ù?ƒŠïβtç?å‡vEœn/?³º N‹?ÔñtÇ#¢?³º N‹>_T1&é>'¦'R`?ïÿÿÿ}¦>'¦'R`4FGL J0618.1+7819¿ê¬4Lùz¦@8ݘ9GIkÀ;#''Œ6À<ÎYáÒ@Lû°>@D.ÛµÜ?ÀY3¢ï®¤¿µ;Šo°*?ð¦ªú-´?ô'ëí¤]Ã?ë8Åû!?¢‰grU¿å]Ðà؝f¿ÓÛ\Ý{›­¿ìÛ~WžÍ?Øý¥²¬OTHERsbg3FGL J0618.0+7819NGC 2146?ï%ÿ³©?"š
ãêo§?›@	Ÿjß?"š
ãêo§?í¯êA}¤q?À]d[4™ú?²€­ô܀?À]d[4™ú?ï9z/Dz ?'âV!.?˜Ðº	¬?'âV!,?ë†õ+=f5?ª¦áˆŒ;_?Áä+S
g)?ª¦áˆŒ;`4FGL J0632.8+0550¿ÄÀ¬× My¿÷*°ãb:ˆÀ:b›!YÀ:ý³çùxý@!Ï¿4ïc@%!š"{$?À'¬î
46¿¸?³ÊnK@üR`õä@>bq`?í²µ)B©¿åèÍÿ|Í[¿í̌€V|Ž¿Ù÷›Â響à³Ü:þُ¿ß÷ë>Qõ@OTHERhmbHESS J0632+057?ïJFäÝ?—m@<¼é?–·?]cdY?—m@<¼é?ì+9ë˜
‹?̯Á¹Ó}?¾¦0£?"­?̯Á¹Ó}?í÷·"¬??¥Œñe*õ•?·XBCbž?¥Œñe*õ•?íÜ
àÃË?§
ņŽ‹?±ùç!ª?§
ņŽ‹4FGL J0634.2+0436e?ì†÷X Ýv¿û4ÂI¼´À7cx WÀ:]I.G;(@	G&…%@Ôó\ƒŽ•?§'/ÞêÝ?ͯº'ÈFÖ@"×\l¡?øá@âV¿Ô(þ;"»f¿Î…:¼êV ¿â†HÿxE·¿ç"O…yQ¿åYÏ^ø]õ¿èxŸN€ÌOTHERsnr3FGL J0634.1+0424Rosette?|ùs¦J	?'IèsRó?ïÆ
³ûl?'IèsRó?rÉ®«¡OÅ?'2»'pÉy?ïÚl¢¨½`?'2»'pÉy?Ðlr"ÜsS?´×}Aûö?çÉƶÆV?´×}Aûö?#ÐK,Õ ?h­ýAô?ïþÂûM2®?h­ýAô4FGL J0639.4+0655e¿×bN)/$?àŸS À7 /^'\ŽÀ9À¡²lÏ6@o½fþ;Û@a&Á4é?´b_£ÿ?ÏÆæxFä@X_^4h½@@í°òý?ïÚ䜸2¿× (ú¿åcÀEç¿äŠ]âsA¿ëÉF/9Ä¿æJe~ßÙðOTHERSNR3FGL J0640.9+0752Monoceros?a¡̅®?akÌ
ª‡D?ïî^ÿé3{?akÌ
ª‡E?ƒr">]Ü[? ;mÉö?ï²5¯ˆ? ;mÉõ?¾ò'ôóƒø?©äP¢¦¤?ì!­¡a?©äP¢¦¤?favÜʏ'?Q¸T¸9ö‡?ï鞉#5q?Q¸T¸9ö‡4FGL J0647.7+0031¿snŒ"Goù¿âN»ßê‹ÐÀ9p°;œŽAÀ;X4Ò@ŸÕŒcûþ@ÀùÅS[È?⡟øXkÒ?ÃÆe¿øS
?ÿ€–"TÜ@‡f$w-´?ïÿhJí¿º¯÷¤ç«¿éºÄöJ¿êÒêRï'¿ä

ù½Ç¿áÓàx"OTHERspp3FGL J0647.6+0032SNR G213.0-00.6?ì´:¼ ?ÀãOe§å?¿^/º?ÀãOe§å?ê#O‹ö?ΛÅìí ?ǓrÁÓ¸+?ΛÅìíŸ?æpL~ò6?·ýqÿ'ƒÙ?Óg"ü?·ýqÿ'ƒÙ?é|JÈãI?±ë$[û¸?ÊÔߘrÛ?±ë$[û¸4FGL J0650.6+2055?çø×:¿œ@"h/"BAÄÀ9æۚÅé"À< öðŒÅ@ úe	.O?û

jKÎ5?¼a%r†Û?³d' +C¦?ûVʗhfò@VX§6?ïðHgwÞ^¿æ¨
/"k'¿Ó6@®ÆÒ¿Öµ@S­&>¿ÖasÕB<¿Þ·a`m("OTHERunk3FGL J0650.5+2055NVSS J065035+205556?ïñãnË?T²2<Ž?\8ý#ökh?T²2<Ž?ïç8•½Ûå?µä@gê?hÇjB$
?µä@gê?ïÁì~›	K?|Ñòڟ=à?	À²{Z ?|Ñòڟ=à?ïJ2q™T?€œY+ö?–¹±ÌÝõ'?€œY+÷4FGL J0709.7-3009¿ïë½?"ÈÀ#J½ÂmÎ:À:—¥ßøù|À<b+¡ƒs@ Šý?ÿGKƒŒ?ÁY:?w9gïlMË?¹Q8½òÐ~@F¸4Õ?ïÿК·¦Ë¿éiüp¿Ô/(âwXý¿ãŽþ "of¿ÕŸ{¿ßއŸÇ8OTHERunk1RXS J070947.9-300901?ïÿ=YÈß?K´°"?]TÆä
–?K´°Ý?ïþÓ>ؓ/?D7•gý¹V?"ÌvÍn?D7•gý¹Y?ïí|1zå?lÙÑ=KC?bƒ÷΅¾?lÙÑ=KG?ï÷uÿÔÿD?@+,ÀìÚ·?QVz!?@+,ÀìÚÁ4FGL J0744.0-2525¿ëJ¯×zú¿ç§ÃÉfÀ8Ï}ÓjuÀÀ;z鳍a@Š9-s*Å@¡½aõ¾^?³ÝLvѵ?Úͳ\cX?@#HÈ/ù?ÿŸlÊX©9?äJSá)¿ÓI }8é¿ÜY"åO¥…¿åßÖÊ|t¿ð?ïÿÑqw;¡OTHERbin3FGL J0744.1-25231FGL J0744.1-2523?r.­=‡"?VµÓÀ[þ?ïÛ碥"ñ?VµÓÀ[þ?‰(÷n…R?®WaÈ1»S?ï›_""Eì?®WaÈ1»S?±ƒ±Þ@.?¦­¬Ÿí4 ?íωÄ7ú??¦­¬Ÿí4 ?FL\yo?=±>?ïú{lèá¤?=±=4FGL J0809.5-4714?Øé՚pÀd]wª\À:
%ÍïâÀ;ÏVØSéŒ@Á…§IZ'@*N뒋?Ã'CeÛQ?ºH"Cnj?õS½vd?ýŖ­V¿ÙT:귙¿×ä[Ê+1Ý¿çý'1ÆK©¿åÈØ\œ8¿ãف±E‡Ê¿ïÿîÝÃÀ	OTHERunkGamma02 Velorum?ïµ'îÊì?|´1ÞRË;?'¶:ÄME?|´1ÞRË:?ïpv-ûšÁ?£œ?–¸?'ñ:@Œ§ö?£œ?–¸?î%îv?kR?ŸóS{œ?­¡œ	JÝ?ŸóS{›?í'ه§N?˜rtk}ÕÀ?³où3Âŗ?˜rtk}ÕÀ4FGL J0816.0-2342?ÍNâήWñ@o4þåMÍÀ:SŠ ÒHÀ;Þ€@J‹¿f\Ö@–Ÿ¸g?ШÄûb?Ó.ƒ€Óz@¡zSƒ5@ˆ`â¿ßRBã)…Š¿ç±/Lô¥Y¿èђ>†x€¿ï[nÎ?¿ïu'>³D¿ïªáö)½iOTHERunkAT20G J081524-233846?ï7ZFrðá?¡e•¨•% ?™·1¡ãÉ?¡e•¨•% ?ä£àü?џ'"žgƒ?×áƸ?Â?џ'"žgƒ?ä=Ô.Ì:Š?·æ(/ˆp?ׄW¢gŠì?·æ(/ˆo?äVӖÐÁ?µ{7Øx–?×éRXÒ^~?µ{7Øx–4FGL J0819.5-3439¿Õ9–ÐÙj¤?ëû=#JÀ9ÕÊÛ[	À;zºÖ*D@ég)ÚÄÝ@":ÚÇa?ÎTð]-Ù?Ø"Ÿ€&@þ'Z·Ü{@¼L0Z;?ëˆÒ!Š_¿Õ(,ÚSž
¿êÒiY_í¦¿èÓÀ§$œ—¿ïþP¤]B¿¤­ÝTOTHERunkNVSS J081945-344215?áµìEfà5?Îki"4?ܔ'u2?˜?Îki"5?ã;fKy+¦?Õºë•]?ى3i
¨´?Õºë•]?àGC¡`ö?·Ž–ü-D?ßqyÞ½>?·Ž–ü-C?ށ"}Ër ?´–ç=«‡?à¿6AF°?´–ç=«‡4FGL J0822.1-4253e¿ìè»Z"ÁüÀ
þ€{»bAÀ7M—üágÀ:ª}ÞR0N@ƒexy?þ"Á-\Y?Ñ÷À&²X?¹Í½7®m@Ìx £
·@XðCõMJ¿Åi€Íú¿Ògáæl¿Þ=êg9 ¿Ü­¤"r¹¿äŠS«x¿.¿âgk*NOTHERSNR3FGL J0822.6-4250ePuppis A?ãlnHh?Êù­›åõ?ÙÁ'×#o/?Êù­›åõ?ªM¨¿'ð	?½ü'=à?î[%t
?½ü'=à?éÒ5ëˆd?²¥ÿ¤-?˼·(QÞq?²¥ÿ¤-?žš™ì†â?…çaE£?ï+3›É?…çaE£4FGL J0833.1-4511e?ëa…²¶ÀÙ0¾
í)À6¿Þ^sSÀ9BY`Äeö@!ägÀ`@QŠ¡¯Ñ?¦¤©;?¡ÙÖ~/
'?ô,Áÿê1@ãhšž&q?æU€e.?ҩ… ¿à8¸¾M<¿Þ¾u5¬¿ç=ñ7¿âµÚPp[OTHERPWN3FGL J0833.1-4511eVela X?àm÷礥?Ò;ðÒ(pâ?ß$1趶?Ò;ðÒ(pâ?ⅸÏ}J?Ø|sLV?ÚôŽajà?Ø|sLV?å̊uí'?¸`'
(à?Ôfëï%²?¸`'
(à?Ð]÷ËBòè?ő_8`ԛ?çÑ^†‹?ő_8`ԛ4FGL J0838.7-2827?çMàÃDÒ@=5¤&»À9"©¥€W©À<pÛs@Í(+˜4??þv9ïå×?³€šëSK?Ó3\£Äì@ïbùÊ\@$ïªGfÇ?ïõT9¿¯ÏÛ Ñ¿Ü{ÔA‹:±¿ÞœÆtÃ÷;¿í­òˆH8¿ïâ."'AÜOTHERbin3FGL J0838.8-2829XMMU J083850.3-282756?nšE†!?k¨!ֆÖò?ïáeº~yß?k¨!ֆÖñ?´"*ƒ?˜k÷¢7u?ï¹/•¯Uô?˜k÷¢7u? ®Šì¸q£?–=0á)Ã?îõQ4xå?–=0á)Å?"µ1§Zÿ?tm¤ó{j?ï­½+9b"?tm¤ó{j4FGL J0851.9-4620e¿æÚÉ6ñÆ¿ó·þ½à¡À6Õ6$;JÀ:p³"&k@!²KH¨»K?üßѧ' Ö?'Jf¢î¤Z¿"¿g€å?ûÄ¿9aK@:=,0_™?ï	H]ç¼½¿Ö©CEO¿âm)c¦˜†¿Ûd`½/þ¿Û±€@,?ú¿È ƒxÅäOTHERSNR3FGL J0852.7-4631eRX J0852.0-4622?íb<}(B?ºôÇ}ÖÔ7?·Ôî½ó?ºôÇ}ÖÔ7?é6ªÍOô?Ô®Yè%"E?Ë%T˲À1?Ô®Yè%"E?èàôB?·®ÖF	??Ì|.÷—Ó ?·®ÖF	??ã+
ŽÛí?ÃZ¾ztsF?Ù©ëòâH&?ÃZ¾ztsF4FGL J0852.5-3123¿îƒ$B¹Ïæ@ ½óùa€NÀ;,%5À<ƒ·'¸¬"@">NÃ9%?ö.­ýÔ¬•?ÑàÙ^«‡?ÏÈžžç?ôŠB®Ñ9C@2õ#Øø)?ïf¿2Zp¿ïÿQ^ÂX*?ïüÉÚ¨X¿Ùoß¡eÀÏ¿Èø»h {¿Ð$—Žý^OTHERunkNVSS J085238-312331?ïûÒÿì–?;H0>µ ë?@´ñM«H?;H0>µ ä?ïù¾W¡
?nëé'$4?Iæ¡{׶?nëé'$3?ïÆù+»"?|ËÃ6As?|ƒj"=þ\?|ËÃ6As?ïåÿD¤ÀI?alÑM¼?j»[?¶ó?alÑM¼˜4FGL J0858.0-3130¿Ûß÷¯Âº@"dj ‡ÊdÀ:^Y­ñ?sÀ<6×%ì"Ó@!±Ÿˆñ֝?úÍwҟt¥?ÃñîšQûJ?·ø™Àl''?öf2ƒ
@!Uå?ïâO`:}T¿ìénù²Þå?'îSžýJˆ¿Ñ«ýI2¿Ôž[JS‹¿ØUd.(OTHERunk3FGL J0858.1-3130NVSS J085802-313040?ïþýüoþP?3@žë?µ?  9úª?3@žë?'?ïùÍBðÈ?gîýj+õ?HÊô<ßçú?gîýj+÷?ï÷ˆ‹ä'B?`''Dò?Pîè6Û{[?`''Dð?ïåIdñJ=?WTQ—vù?j¶›µÃS?WTQ—võ4FGL J0904.7-4908c?íŽÊìã_¿öú@óæJÀ8ÖÞZ"ÊÀ:Z¿»lR9@\´5ý@	STÛúg:?Ð@rM'À?ß݊àY@ŸÖjÛ@@j>NX(¿ìîàwW?ÛO®~ƒÄ¿ëU£ ƒ˜¦¿êÐäôá¾Ì¿êž–Xœy¿ïÿG]â‰MOTHERunk3FGL J0905.6-49171RXS J090505.3-4903244?☡ۜ?Ó.
xPî×?ÛðνÂHÉ?Ó.
xPî×?Õ}¦b"´?ÌԒ=¨œ?ë –gZÓ?ÌԒ=¨œ?Õ1g©cÖw?µ#Õ݂Æ
?ågL+NÅ?µ#Õ݂Æ
?‡²_^æH?z ;Ð:«?ï¡6'‡ f?z ;Ð:«4FGL J0910.0+4257¿åpï
Åp@EvFbºà;À:i—Sn<À<{8bG@è!©s~@<¡pþp?ÎêÒñ±‰?ÓЧ¸@MÎ@5@%Nn@·'ŒYë?íݻŽZv¿äðÄ"ð¿äÅõãF‹Ö¿ìÒÏæ\ÀË¿ïì¿EûŒÔ?ï¦ë\ÕOTHERcss3C 216?îžáÅŽ?¨p{А.?¦ã®Þ'?¨p{А. ?î´Ø]zä±?¶÷£-;o?¤²z(Q´ß?¶÷£-;o?ë0±Ï'"u?«XO³=Ë?Ã=8Áµ®+?«XO³=Ì?íøøy#~?¤ç v×¾?·8<6ä?¤ç v×¾4FGL J0912.1-6449?êò\QXÄÀ&n8§ç:6À:œJNìÀ<=²ôݍ@u±ô¯>ò@‡È
±™?ãHv;?Ê#ðõöç¨@æ;ƒcÍ/@)åËv`"?ï^·E|¿ÃjÓÞcøù¿ãíŸ
⵿ä`³Ô®Bž¿ìª0À',¿ïè,9CîlOTHERglc3FGL J0912.2-6452NGC 2808?ß<ðŠbF?ÈzqòÍ6?àa‡ºÎÜý?ÈzqòÍ6?éq™Jqƒ?˚ £j2È?Ê9š×ª9ö?˚ £j2È?ãnà½/?¹îèDo}?Ù#â>…¡×?¹îèDo}?èä)á¶ü?«p=q5?Ìo[üy$?«p=q54FGL J0921.7-6317?áøäžèÀ"Í$žDúÀ:÷I,™»þÀ<¨p˜ïO¯@µÃvâµl@oÿ^ðP`?ÍbvAЯÛ?àÆýòÿf@}ñ'Ž»?ïþޔY#¿ïýSõËÊ?ïÿ¢­>'¿Ø†±_ˆü"¿áÔêp6Ê¿ïÿâÙ~‹÷¿¹à—/'âOTHERlmb2S 0921-630?䁹êÉ?ÌFa®·?×àüŒ*mÛ?ÌFa®·?Ïbpàú³?ӒÓˌ¥?è'cùÁS?ӒÓˌ¥?ͦï0´?µ'å¤=À?è¹D3Òû?µ'å¤=À?§þ›ÈÅ?'=®‡>?îŽPOÃt?'=®‡>4FGL J0935.3+0901?¸&S%íd@D1'€w‰¤À:&<ì™.À<‰w¦×@	ÌžT@êû܄е?Åˆ¤~Ïê?Ӌ'Û9w@
¸«ôÌ@Ûa:,¢¿èÌ~=šZ¿Ð§ýàk¿ãèÖt¿ëp×£Àd	¿é g´D?Ë¿ïü²ÙÀ3OTHERbin3FGL J0935.2+09034FGL J0935.3+0901?âtªðçp÷?Í!ÿšïîé?Ûª1?Í!ÿšïîé?ï7…ðu8?²ŽfIZ?™AñXÿç?²ŽfIZ?ᢲùЅY?¼"Bœñë?ܺš^õN?¼"Bœñì?ì›ÙýD?¡']ˆxq'?»!0¥ßÅ?¡']ˆxq'4FGL J0951.7-5328¿ª{ø.S€C?àœ2#iÀ:,F)¯ü²À;€U&£ø@ *úõÿöñ@Ï=ÀTïF?»•«ß}´¿·tA4A•?ùÑ(çÖz@o…'Ñ~b¿ïÿKâCW?ïø›AåR«¿èí][zпÜÅåNë ¿æ—â?$Øý¿ßFôçôOTHERsppSNR G279.0+01.1?ï>M­üøw?/±´õ?˜6J@`ñ?/±´ö?æd5÷f?Öf°ø?Óó6Ŕ1?Öf°ø?í¿q%ËÊ¿?¤¸sÿw7?²vÑ¡ª?¤¸sÿw7?îwZ™Åß?™Eˆ/¯Ò?¨ŠVc¯â?™Eˆ/¯Ñ4FGL J0955.3-3949?ïGå¼Ò@'ì9yžRÀ93"P>ÝÀ;¦d—YMy@³›­E@óþ?¶=̀{æU?Ñ¥«`@‡…@ñ'©"á@THV±?íêhô¶â¿ÜÞdå1óm¿ä†2Ÿ£‡¿æÆŠÁX¿î¬­½½æ*¿ïÙî§z-OTHERbin2FGL J0955.0-3949CRTS J095527.8-394752?}ŸÇ'/žš?~D2µ^?ïÄÀpû Ã?~D2µ]?ŠKw˜6`?˜½ÐÃ~®?ï–Ò!Ÿ&}?˜½ÐÃ~®?À^¬ìf¾?«o3©¿™?ëèTÄæP?«o3©¿™?¡Ö0üìÈ?Œ¶dÞùwO?îâœð6ñ3?Œ¶dÞùwN4FGL J0955.7+6940¿ïò²P?=@DH¼ƒ©mLÀ9EMÐÀ<_¶Q`Dä@‡•;;~@[­}|,¡?¨Ù#ƒy?®ø¤
]X@ç*ÙÈ]Ò?ü֘UKáÖ?ïÿ ~æ¿à+RÿTÿ¿á¶Gº©´š¿äß=¾.¿ã©<"?¾¿ç«S€Z®LOTHERsbg3FGL J0955.4+6940M 82?ïÒZrÁs>?tv詯˜;?vÒƟF`—?tv詯˜:?ç€6å*?ÔA W3¢?ÐÿÅù'5¬?ÔA W3¢?î£!à^Ý?š±½QÛ=?¥Íáú.ð?š±½QÛ;?áŒÍlXq?½ÆñéuÙí?ÝÖæe'O?½ÆñéuÙî4FGL J1008.1-5706c?êAh}xN¿ï<Úa
À8¥1G ¨'À:,Þ¨@¿¿>™Ä@>	»j¤º?ľ>ÿðÈ?ÀÀáÜÿIø?ü1¸ðiŠ?ûëøŒR?í'ÜEæ"¿ã°¡óÛ/¿åº &5¿éÜo6ï€V¿ã{ÕctCŸ¿îës`OTHERunk3FGL J1008.6-57061RXS J100718.2-5703358?Ց?Ðq‡1?ЎÈ	î"ß?å7`Ç<g?ЎÈ	î"ß?áƒðE•œ?ÕiÛíü¤?ÜøtÕÎÇ?ÕiÛíü¤?×¼FzúÓ+?ÅŸDZº?ä!Ü'–j?ÅŸDZº?ÄÁÊ3á2ç?²aݳîèÝ?êύs³G?²aݳîèÝ4FGL J1011.1-4420?Ê7£_ª@#b'è},|À;2*߈'À<‰3úÙO'@ "«#Ú¦?ÿdž!Ðý?Î['ãG¯?¥ñïñêém?Ý'½†,@¯»ù9¿â˜éÛÑLŽ¿ìez]"/Í¿à¶@º°@¿áñ–`)5ƒ¿š¢ža:¾©¿æÜ¿· ìOTHERunk1RXS J101130.7-442241?ïûmm¤'7?<å¯õÀV£?BJIm»%Ç?<å¯õÀV ?ïüXjìÔÒ?`öŒt1¨~?=<¨™YvÛ?`öŒt1¨{?ïî锗É`?iÁü%Ç;?akh6Ÿ€?iÁü%Ç*?ïùG÷m ??Ó[s\)y?Jãœ"K'Â??Ó[s\)n4FGL J1018.9-5856¿¤¶\ñ‡¿úõ<WŸ#FÀ6*OÁß3À9­HJ­@øhÑz±w@rÇZˆ?•0£¥XŒ?Î_
¼òd6@6]3]$žE@/È´²¿ÊŸiKs¿àm	]¡Æº¿åyöÁgéÉ¿èàÓ¿Û¿í#>=ÓJ?¿ènq—òÐmOTHERHMB3FGL J1018.9-58561FGL J1018.6-5856?icG.1Á?TK|²?ï朸èÑÎ?TK|²?PG¯Øý©?bKŸFžú%?ï÷Üx(?bKŸFžú%?®wiIߜ3? ß×£Gå?î‰kb<? ß×£Gå=âµÅ6È´9=òö\üŽn?ïÿÿÿíJ;=òö\üŽn¤4FGL J1023.3-5747e?ºÐj~a£ ¿ÚDUšfH3À7×xFÜ]À9›mjW@#_Jé2^@v¹<Íé?¶éπËf¿j&¶Ý?¾50¼ê¾@"Ǥſí(@éÈ?ïY¯¾ôòÜ¿ë[¨«¿ânŸð˯–¿ã»>U¦¿ÛþĖe×OTHERSFR3FGL J1023.1-5745Westerlund 2?ܽº§'Ç?Ñ툋N…?á¡"ñ,7?Ñ툋N…?åæ°9å?×±ÌsJÂ?Ô3ʟÌ4?×±ÌsJÂ?ãp׉®íL?»ºLF{»?ÙPì¢%h?»ºLF{»?â¸e
"´s?ɜgãú:?ڏ5êؗ?ɜgãú:4FGL J1023.7+0038?{ZH@Fä'úòÀ8Dœ¤æÔ¶À;ýÖ.u@ÿªó3=ð@Üb¼ºh?¡žÞÁ°¨Ä?Ç.95×@"2¹o!öË@½€šFM?·Y /_éõ¿ßa}H€!¿æ†_€>:¿èÅB>éË¿ì3ŒŸ`-¿ã'?´‰	OTHERLMB2FGL J1023.6+0040PSR J1023+0038?îB‰×?©žAŠ¬`…?®ÏžK×b"?©žAŠ¬`†?ïæB˜[›?~ïbòþ?i½g¤d?~ïbòþ?ì³élN9?«ݳ0?¿
`´Ž3?«ݳ0Ž?ïݨ¨Tµ¨?c`¿B%d?q+«Õ¥,?c`¿B%c4FGL J1024.5-5329?è¸j÷"æ@
çDñ¢À;1#³co;À<']9—@"?Öê‡ô?÷‡åÂg=?Ö=…³:?ÞAãd¾Æz@	0)®O3D@™zu<¿ïÿþøþ"¿Ê0™Ã?ïÿTßUe¿Á¡;#—Š¿ÒUÖ¿á±÷(ÀéjOTHERunk1RXS J102441.6-533141?ïÒi¤^.H?sòö,
Ÿ?vË-ÐèÛð?sòö,
Ÿ?ï‰ëÜs,y?­
žµ6?…ã4á×?­
žµ6?îۏ³°š?—õӌHÈ5?¢O·Äöd?—õӌHÈ6?ïGŒ®«Â?‰&©$Ëі?—j>Š‡Ó?‰&©$Ëѕ4FGL J1024.5-4543?ÄÃ|±œ@#Àd©ÍÄÀ:´úŽ¦÷À<qZ»7y@ êÈÓmû±?þ"ä0—?Ä0³|Õ9?ªZÝ#å•ú?èaþÂé<@_£Ùäbk?ïéè »6w¿àN¦@Æç€Ç¯;¿Ô]´;0'ª¿Ñ¢5Ÿt$¿ãµ\"•¬$OTHERunk3FGL J1024.4-45451RXS J102430.1-454401?ïûk‰*ê?:GïˆZ½?BQÛTV?:GïˆZÎ?ïöœ¾²ö?oËý¨ù;m?RÇȂš??oËý¨ù;o?ïî5ý½yÃ?j™…šË?V?aÊB†=o?j™…šË?Y?ïºv+Â]ÿ?i½¹.áy?buh€;?i½¹.áz4FGL J1029.3-6657?éÈ咡ÐÕÀFr*rÀ:…úcÞ̪À;ñ讪¢Ö@ŽöÑX!Õ@WWÂHå?Æn=à¶8·?šOãÃ?Ø-™–>›F@Ï#¾Ì?ï
–V:‰¿è¸…íë*†¿êŽ
>¬ãù¿Ý¬ºÞ¿¿ã›â´•žb¿åPT "žXOTHERunkPMN J1029-6656?ïûÐs½{?B¾²õêŽ?@¾1
¿?B¾²õê•?ïþæ€&»?C됱͕?!—ý"NÚÔ?C됱Í£?ïÅlü]¨?€*Îíì?}IðÑ+Ä?€*Îíé?ïøÝ«w¶P?9'}o8@?L‰R!&¾s?9'}o8I4FGL J1034.7-4645¿î3U±@#Û,B»fÀ:ïùZÊPòÀ<cÐÜ&$@"pçɨ@'}ô!¥?˵Ï_‹+? ¿5#g'?Ԇ$¼øÄL@¹9õš }¿¿'£ê¿ê±(+˜4¿Î§!—¿æ]gÿî<¿ÊçFu°0_¿æÎbß\\OTHERunk1RXS J103438.7-464412?ïüí6J°?=òEÛF??À–Mª'r?=òEÛD?ïü,Ýjo"?b)aGó?>™¬ƒÜ
?b)aGó?ïãã_¸ªN?rø ÷	³ð?l GU²g?rø ÷	³ð?ïú<âPl!?8'¯HÆZý?Gv¾Oz¬?8'¯HÆ[4FGL J1045.1-5940?"߳‡»ˆ¿ãüpÿFœÀ6høj	‰À9êƍîj¬@î«Ä¿b@©²=ÕM¥?'Šg!¢<*?¼Ø;•ØCù@'Ú^±¬@¿+½óëö?ï(Åñç9¿×q10–v¿ãì2žðÔ¿äTµÏZEÇ¿è°&äpX¿ä¹Ùk€,OTHERBIN3FGL J1045.1-5941Eta Carinae?Ç©õk]^­?ÈgNI§ß?ê'¥(¨T?ÈgNI§ß?ŠèÓm´Ö"?¶bÇaÁL?ï"\²I,¦?¶bÇaÁL?åþ›;oÙ?³þt Ù ?ÔÉÿ‰ M?³þt Ù ?2È2,5?*øð+ÃS¥?ïý¦ùº}q?*øð+ÃS¥4FGL J1045.7-6414?çIiÀ8úÀ'C{À9Ϻ˜í¢/À;¼áG®{@báK´ß@"õ?²w?Ã>ZÕÈI?Æl–\ò@\,CTéf@裉1—}¿ïþ¢˜›Ã?ïúiˆYÖ5¿ã÷M©Öþ¿áJ·~†îœ¿ìSá~Š ¿èú˾!OTHERunk3FGL J1045.3-64141RXS J104537.2-641438?ì¬7oÒd?»Ûᐲ]?ºžDoŒÜ?»Ûᐲ^?î@¨)Tš?Àcûzx24?«÷}j¶W?Àcûzx24?êQÉq¿D5?²b@i'ç?ƸÚ9ï/?²b@i'ç?ìq¬C
Åò?©®FWÝ?¼rç'Ðq?©®FWÝ4FGL J1051.6+3253¿Á9íbI@OÃ˼+"ÙÀ;'?Ï"èÀ<êՌŽï@û´ò»sß?ÿ†YJôðØ?×ǘšëÿ?©	%B¯¨?ѱÁ"õxh@BÜÔ+æ¹?ãxo'Á¿ïÿôw5Áƒ?ïýއà3²¿×E;ÿ	µá¿Ô—Ø"¿ïÿe`õäOTHERsbgNGC 3424?ïÿªfì?B
"™?úæEÄ?B
"°?ïý¨1'Ï6?K‹‹ÌÖ?2¾si†J¶?K‹‹Ìå?ïò"ɽåª?i)㎆©?ZÖl"4«N?i)㎆¥?ïÿzˆÒ€½?mY~Üù®?®å¯è]Ã?mY~Üú4FGL J1059.5-6021?ì#%Ë!Æ߿ܾÒ
SÀ9³9ä'À:š>—ëC°@lTi¹­
@ªÂT£Æ?ÊäÑ{]C}?Ï$_ZÙjj@>ä\5Šü@2\sž]?ɖƕüA?$Ç/¿âa4x­'¿æ¥'ßæÚë¿ïÿýç!é?ïÿ·pD5ºOTHERsppSNR G289.7-00.3?ËÈhÂûkÁ?Å፳ÚV?é
åÏA%?Å፳ÚU?á-馿f?ÖhP6Ýe?ݤ,³ü5?ÖhP6Ýe?Òu¬Ï¨H`?µQ®ðhôN?æÅ)˜+ÛÏ?µQ®ðhôN?ØR­Dè0'?¿«{Ê8)?ãÖ©]‹ç¶?¿«{Ê8)4FGL J1114.2+0638?Öiªþ±Yå@M'ËÿGs\À;¾vÌ7«À<Ø'QT†@"_©mø,?ÄWoRž2†?åÄáçDò?ïûo! ä'?þ8¸É	É­?ø2¥4M¿éç÷Ë~4¿ïÿߞ¶Žó?ïÿ.´Hq‰¿äÑq5Í?ʌ3)£'¿ìYƒ)Ì@OTHERgalIC 678?ï­5§1à—?‡*(˜¯ˆ?"²–3‡Ú]?‡*(˜¯ˆ?ïôȞ»¿?']ú["µ¸?VnÃĈ'"?']ú["µ·?î°ü™ã¶–?—…÷ •Í?¤ð6aĖ©?—…÷ •Ï?ïÈçîøv?oљ
ÿ?{ŒñƒÅP?oљ
ÿ4FGL J1128.2+5831¿éè›֞T@K¶-VÀ;b°+¬VÀ<ёúhçJ@Ó£åLöS@îÛŽ,?Ð{uâZR²?¼oa^®?íÝe k/y@Öm¹kñì¿ãPxˆ§ÙοévýÃÝé¿ßäY±L¿âmf4è?¿ëўJÙB?Í×͜U‹£OTHERsbgArp 299?ï÷xÃQ'þ?QÈoKˆ›º?Qy\Ú?QÈoKˆ›¸?ïüEâq?cY:Ûlš?=ÐïÜ~W?cY:Ûl›?ï—æÑêFD?‰£Þƒ~F?ŠK…nné?‰£Þƒ~F?ïænc¢ô¼?Xí—sSí?i'œ]Cy?Xí—sSò4FGL J1151.4-6248?劸'ã¿çz¾ï>'À9!JÕh-À:À´†"éß@'éçÆ²@ê²ái<?ÂøScTc/?±¨Ã
†P?õ§ðª!§@²™Å¹?Õ-GáÀú²¿ßø€‹*Á¿ê¾9÷r'Å¿ä"ô¿7G¿æV‰äð°¿ëaÚ`3F~OTHERsppSNR G296.1-00.5?êC`·oŒ÷?Âk#DÙe6?Æò}"AÌ#?Âk#DÙe6?êaQ'ˆf?ϞH|,V(?Æz¹õÉÞc?ϞH|,V(?éz:«Iƒ?·XËVx¤?˲RÙð?·XËVx¤?èð¤ÍIØÊ?±ù½_	û?Ì=lÊ؜Ù?±ù½_	ú4FGL J1152.6-6207?å÷u *â࿛N(¾ rÍÀ9ÕrQV3éÀ;€ö4¥#@åQ(À@%iF·G?Ô: $x/g?ä{àK.Ò@Rµ¼åÎü@Á'kՑ¿é%÷@=ݱ?®T˜€uv¿æbÀi'¿ë›[Õì¿êC,oʓ7¿ïÿü¥¬¨OTHERsppSNR G296.1-00.5	?§°F†"<4?°0á̙m?î"û—–Ì=?°0á̙m?ÉÙÁS·_¾?Ђ‰]%?鉏«(?Ђ‰]%?ÄøËm?«Æ:â'¯?êøÍ$»?«Æ:â'®?¸Ey'kN?¡ÕÝLŒ?ì÷^Û–?¡ÕÝL‹4FGL J1155.2-6259?ÑçÅb/Ä¿éè:ÛÀ9'6TOãmÀ:—yóáäŒ@"éµæ¬G@¸5u-?òƤ^ïy ¿îL?á&£7¨ú@Öð<=ž?ß¾Y¢2ÅO?âKÕážk¿ç˜}Ú÷1û¿æ/Y‰ß¿é«^½ûx²¿æÓ¾ŽE¨OTHERsppSNR G296.7-00.9?ÝɪF{$c?ѝ[[e?á*ÜÂmÏ?ѝ[[e?çx*%0zX?Õé"͉j¤?Ñ«µŸP?Õé"͉j¤?å#Nìì?·wLŒõ­?Õ¹Ûb&Þ)?·wLŒõ­?è¤ç¹¨ÌÓ?¿}(MÎ?Íla\̲?¿}(MÎ4FGL J1155.6-6245c?т88Xÿâ'óøŠÀ¹À9+û¤P¬ÁÀ:lE(þüË@Ö*%mwÓ@íÍÛÀ…—?ËJY™??Ñäg¾U:Å@‰óžÈ­ƒ?ö'ÞÉN"¿ç€E4½vî?熁žü?ŠºDΪâ0¿èÒ­N ¿ëfÖ-¿ïÿõEq#OTHERsppSNR G296.8-00.39?³ý1Š?ÀtîSíøE?íà\ùμ?ÀtîSíøF?¥Pùöí,?¶þQ¿¼?îªð`'->?¶þQ¿¼?¸º£Þîb?¤@U­
W?ì諄"<"?¤@U­
V?ƒÂ!ün?t¸Š?ï°÷xGÆ?t¸Š4FGL J1158.3-6232?Ÿ±'gÚyä¿ÒØ>e@v"À9)Þ®v pÀ:½¨ö-ï'@ XQÀ'ô@Jh˜q?Çm™I'›?Äug5CXÅ@nÜV­Œ@»{–¤G?î"ßÄK¿å´—1š­¿æÂB/Oy¿çñ§w¨®¿ë­ÌŸJ¿éë֙Õ)OTHERsppSNR G296.8-00.3?êµ±x(Ä?ÀD!ì™H?Å+é:\ô?ÀD!ì™H?äÇßȋh?ÖP˜Cª-?Öp@néÕ0?ÖP˜Cª-?èR"Xüƒ‡?²}tèÄ
¦?宜
ñà?²}tèÄ
¥?åµ*eïÊ ?º¼ª±Ì?ԕ«4 jÁ?º¼ª±Ì4FGL J1159.3-6122?ÂGÉ{öõ(?ëýH•›À9Öƒ.ô	À;šCㄟ@Jö‰‰¬@¼*`%څ?Ì)ž‰îUß?ÉŌ§Ük@_î¥d¨÷@dHÔÛ.?æüóÁ-\Z¿Ø¶ßz¤`ó¿á-ÆwH5ú¿æQ6É>£¿î	¡Ñv¿ïþÙú²¹%OTHERunk1RXS J115843.7-611934?Ùøì3'Œ?͆pƒ­?ã‰æl?:?͆pƒ­?á|tˆ®¢ú?Õ&FÌK?Ý?Õ&FÌK?ã`ƒº…+?¹oÌçØ?Ù>øŠõ©á?¹oÌçØ?æ€éÕr
Û?±:Ü^Ìåò?Òþ,UêH?±:Ü^Ìåò4FGL J1208.1-5149?åog¼M6f@$ô‡Tów\À;t2À<kAHŸ¬@ oÔn+ן@.Ʊ?Êœ§@ W?¬éᅖ'c?äõ"FK=ì@9ʎÙø?ïÿ¢­>'¿é̱‰zg¥¿à˜Øÿ`ö¿ÚJS`OK¿éÃsݝT?ÌtÀÇ/ÿÍOTHERsppSNR G295.5+09.7?ïý3š6?:·§Žd?6c.Oï(]?:·§Žcõ?ïú_"Oo?l&OÇ<tc?F³ÞÂEB?l&OÇ<td?ḯ•Î«¹?~Y5Éÿ%?y¿5ª"æ?~Y5Éÿ$?ïèŽDʨ?U¬'97à?gq»ä5Xœ?U¬'97ã4FGL J1208.5-5243e?ßyðä{¢@#0FÜ]dÀ9#V›‡À;ŸâV¡ÍE@ eSµø ?þÙû‰xº?«¬=
LŠ?"XÖʖU†?Üyb—yÚ?øˆmÅ*l?ïõ΃†1Þ?ïŠIˆà¿á÷=^ZS^¿Ö&Å#
F¿àêâ«¿ØÙ	Üwº¢OTHERSNR3FGL J1209.1-5224SNR G296.5+10.0?ïØ>X8¯?nâ۟µb2?sàÓã¨??nâ۟µb4?íR]ic?Ç:öQöÃ?·m´ä?Ç:öQöÃ?ï+ÛÎuš?"Pg¡úU?ú"†1L³?"Pg¡úV?èý¤-ä¥?¶:7íåìç?ÌùoHmo?¶:7íåìç4FGL J1213.3-6240e¿ï¹@óX׿À=çՒïÀ7@)íÀ:,…dž@™bRZ•Î@¨]Ywj›?¡‹:ÜúA?µXè_¶…@lâ¬2#@z$b_ñ'¿Å¥'Abv¿ÕàQ<¿ãyâyÝ;°¿äv†¤ÊOD¿ç#ĀM`¿ãhë¡y6ùOTHERsnr3FGL J1214.0-6236SNR G298.6-00.0?ÃTƒ'™^?ÆdK§rê?ë*ßY¾(?ÆdK§rë?‹VÇÀ»©H?žo"‰$àü?àýZ?žo"‰$àü?áv%ìiœÆ?»-§ÍWv?Ý´',Æu?»-§ÍWv?‡N­{irs?vðÒO–°5?ï¢ÅJZ6?vðÒO–°54FGL J1256.1-5652¿Ù‰hõ»¤@ùú}	@À9Ð)é•öÀ;¤uÓÁ³"@/=;tË.@"|tÅ¥?Æ-+²5qÒ?àD@÷–û@{xÎø?ø=ìl¥DÉ?ïúÂT£Æ¿Ú%›eK´3¿é1¦€²Âà¿ëxöLÖó¿åŠºÙ…Aô¿ïèP¶Ñ¸ÅOTHERunk3FGL J1256.1-57031RXS J125554.2-564945?Óךav3°?Î@9ïv?Ž?æ2ÏDæ)?Î@9ïv?Ž?Ʀƒn,Žw?Ë%½"·.ˆ?êV_$tÜb?Ë%½"·.‰?Ù[$º3à2?¹ÜsÀ¡ðÁ?ãRm¢æç?¹ÜsÀ¡ðÁ?³;Ý
œé? ~ÄÉ5|ü?혜D^Lb? ~ÄÉ5|ü4FGL J1302.9-6349¿ëzðtTÚ¿ï"ÃÀ8Ôðý-½¨À:Rj¢Ž5@;ó HŸ×@#v"Á›@?µåš¡+‰¿µý 1
i@\[›1IN@î1·?ïÜ<a/Dç¿êUÈßWhó¿íÉÂVQEm¿àÚ!2Æ¿ædÆ®0*?¸iE~d^úOTHERHMBPSR B1259-63?îÓLZÅ2´?¬7èñ?¢Ë:S¬ÔÅ?¬7èñ?ïý:ÃÍÙ?hP̛N?6/áá'5J?hP̛N?êü_=£ï?¯»mÌà:W?ă	pC‰?¯»mÌà:V?ïÿ)¸æ<z?ti> ?Èã8pÇÅ?ti>4FGL J1303.0-6312e¿ìDOÈõ¿ÖáU…m'«À8EñÓò[À:ҕˆ'á@"'|2iµ?ýÚ8
2ˆé?ªO"›Ø¿£e">=¨W?÷ˆ•âU?ûÈúDÕ'?ïh«…Th7¿Ø6rûé¿àÛ?÷fÔJ¿â…`\a)ç¿Üíaw¤Q¿ÃQu¾sÐOTHERPWN3FGL J1303.0-6312eHESS J1303-631?îòêÛðË? µ Ì0½Ï? ÑR@ÿL? µ Ì0½Ï?àü¥"¶Á¬?Ù&Ÿtªû›?Þ´ö'|§?Ù&Ÿtªûš?êäEØ/m?±•ÕVeُ?ÄnèŸBKÏ?±•ÕVeُ?Úð}ûZV?ÂlP\ŒqŸ?â‡ýÁRÕ?ÂlP\ŒqŸ4FGL J1305.4-4928¿ë€~iYM@*«h'0ÆqÀ96s¾=½ÑÀ;üR$A@Ò@VÝ1t@êù>?­7›!Ùïu?«ì^Ó¶²?üuÞß)@¥^¿þÞ?¹j£Œâ|¿Ø¾U{1¤"¿å™ç'Z¸³¿á¾'¼ÞB@¿çpÖAj®u¿àâ~å¹-OTHERsbg3FGL J1305.4-4926NGC 4945?î‰ëô™ê?¢¢§'|š?§aO¶a]?¢¢§'|š?îB£gŽ›?¾¸«A‡G?«ÕɇH?¾¸«A‡G?±—…?œ‰ªÔâ®?¥¿d懱?œ‰ªÔâ­?ìó=t¬§? †>˜3·}?¸f[òšÅ? †>˜3·}4FGL J1305.5-6241¿ïz=]|~?Á9Û×À7Ù\M}À:\Ê4lW@xƒ
¼L@ãö<1ßv?­R°Å/J?¤§Q"¤q?öéëÜ\ŒÉ?ùÒ¼­ð¾š¿Øž½ûx±Ã¿Ú)²ÒÛ¿âþtàÀ˿㕮Þ]¿è¨Ÿ%ʔä¿áýiíÚcŽOTHERsnr3FGL J1305.7-6241Kes 17?ϟڂ
ÆT?Ðwè.?è	_|Žj?Ðwè.?ÒÐ!<C	?Õ.Ƌ4¦Œ?æ—ÀoaÞ|?Õ.Ƌ4¦Œ?áßǁ®1?¾–;Äg/?Ü@pü¢ß?¾–;Äg/?ÐÐÑ.T,?ºý¾=ì?痗h·Õé?ºý¾=ì4FGL J1326.6-4729?×?·9@-êy5v'À9C	A}À;å±^²<ÿ@Û¶ˆÜÌ@KÌå €©?´"=l@?àùíÌ÷"÷@'eØם
g@PôF¹?ïdC¬':׿ÔPá_ø¿Ô¦êk²¿äè+Íä¿î¯4¬¿ïÿÿ" 5•OTHERglc3FGL J1326.7-4727Omega Cen?M»€ã"'?Rš1<ù™ä?ïø':ŸÇ?Rš1<ù™ä?k¢Bcpž?yÕ£Àº?ïä]½œë?yÕ£À¹?‡3ÒR…'z?ný-¸½,?ï£0¶µëb?ný-¸½0>ý)ù	—ë¦>õ2&*Î(?ïÿŬ
ìÐ>õ2&*Î)4FGL J1331.0+3032?ï¡5lŒn@T+ü27‹À:ւè},|À<›µäRûP@ž&ÂaŽæ@ŸŒÝÉtS?Ç`ñ\y'´?ÅüÚ܄ü?ýšMÀg?ü´P^è×?æ)ÖÈÏK¿çñ¢ÚŠûq¿ç`Á`ÝæP¿ÚOó]ZN¿ì°-…C¡¿ïýM"ŽÇOTHERcss3FGL J1330.5+30233C 286?ï7uí3?š
³x`U?9BYž?š
³x`U?ìÛÜ¥¢É?È¢íÈRÊ?¿	!Òéº?È¢íÈRË?î³î¤ò?™8O±
¨?¤Á°Ö'5?™8O±
§?çCÎì­zm?µQ_Û2y¥?Ñxb&¥'?µQ_Û2y¥4FGL J1343.8-6208?Ú߂ìƒa?»õ|"š7À8ƒ%{º‹'À:E×z¥¹@[#¨üŽ@ö"|#g
?ÆGX™Ÿ"ð?½|_LØ@-wœïo?î~՟ž?î|äù¿ÒŒewS¿æBaP™¿çÉâ!GÎK¿ê	ÿ\–¿åì†;OTHERsppSNR G308.8-00.1?ÓÖà²;?Ö`|ÿy?揦ÿýb?Ö`|ÿz?Êd{o´ÝÝ?Ñù|n{Ë?éfá$ȉ?Ñù|n{Ë?ÒÇ,òYö?ª&ºÞ·?æœiôÓ?ª&ºÞ¶?ŽñÌráÙ
?|—WœH7Þ?ï"8Î4xœ?|—WœH7Ü4FGL J1344.9-6228?×P~}‡q¿ÏnëE2åÀ8¹ŸœÞÀ:4܃ùõ$@è8<ÝV@‰ÔDRÉ?Å¢ÁvŽö?Ý[ÔýrÜì@ìý
y@,:Z™Ô?ãH¶‡æ鯿ٕ˜ƒ$"¿ÚMy£¨¼¿èˆôe˜
M¿î¦âÂØWE¿ï×ÁÝÛgðOTHERspp3FGL J1345.1-6224SNR G308.8-00.1?7ü¯u³e-?1©Æ.œÖð?ïýjI"?1©Æ.œÖï?†3íúo%å?2pΛ†¨?ï§0HCh?2pΛ†¨?ˆ4²°?l¿\ âžÎ?/Å5??l¿\ âžÓ?`Þ|MFð?NLæÉ ò÷?ïï!ƒæ²¸?NLæÉ ò÷4FGL J1345.3-6253?Ú›4޹пäâÙÿePgÀ9L[[piÀ:¼2JÕç@^WÏâ@ª*sq?Ïý‰˜š–?Úò²Ú³?]@!móùa€@óI€Òx]¿ïñ7æ Zé?ï•dSN\¿á`ÊžUì¿ç{wÀ*ýÛ¿ïÿÿÊPË?ïÿК·¦ËOTHERsppSNR G309.2-00.6?Ç	sO¯4?Íô7÷?ê=£,"3?Íô7÷?Î3Ý(C]?ÑrûgN?èsµï(¸?ÑrûgN?Ãv`wˆP‰?¯~xA!?ë"gâëÝ?¯~xA!?è-(ª!?³NBç¶M¬?ëôµüUy?³NBç¶M­4FGL J1355.2-6420e¿Ô(é°
™åÀ•;›·À9¶N¼üuÀ;w™÷j·@%tÁ¾¢h?öªî «†?¼wbâù4	?§¥C_¿òã?êyÔ½\@UaµQ°ø¿ïòl~®[È¿ïì "ÚÅ´?é•\¾Fø?ïýaw]¿ÙÆ|¼A%¿À]GóÐGOTHERPWN3FGL J1356.6-6428HESS J1356-645?ïú¥óE?AiH¯,×Ï?Eh3úé¾°?AiH¯,×Ç?ffi8Ïû?°PqxSÌ?"ß1Ì<Ý?°PqxSÌ?ïh§'à?•hÓK\'?œRý«
Ãî?•hÓK\'?ïÅi"\"?}E(Í?}K6Q¹6È?}E(Í4FGL J1357.3+3730?•ü}É·C@R+µ^ñýßÀ;ÂD—Å¡À=ÅÉ£L¡@ k°'­¼ç?û'²z;/?ݲ~ñ"?ÔP`j£âÉ?ö‰ì˜D/?ú(¥é34á?åŊƒ| ã¿í]ï3ÿáÍ¿È`—D€¿áY+€Á¿Ôãr@9V
¿ïþëbº	|OTHERgalNGC 5380?ïè±ýíq…?hýÒaß?gNŽ{£?hýÒaÝ?ïðÊWEc"?xfvgpÀ?^kQu8Ùd?xfvgpÃ?ï=õ¤}?'ÞoQ5'?˜\Kp\Ù?'ÞoQ5'?îÊ{ªWp¹?'ßEƒ‰)?£XEZˆôj?'ßEƒ‰)4FGL J1358.2-6210¿í¾ùK^Ú¿ÓwÂäì~CÀ8SÒkr>âÀ:WoÈ@ã'4pJ@[#<E*¬?»5€•f¯?Ѭ‰á?Ër@íwàmò?û'ºz9×è?êœâß]É	¿ÛÖqüœž1¿ãŸÕÞCl¼¿è±·Ÿ¿ì踻Ð`¿ïýáÃÔ×OTHERsppSNR G310.6-00.3?"T__ƒh?±¬Æ[Œ³Æ?﯂®'ò?±¬Æ[Œ³Ç?N
Fu? BؘnlÑ?ï}¯ó•Ì? BؘnlÑ?Œ%·h?~?CËx?ïi#æ_·?~?C˃?cP ¯Š'?Pôkø±f?ïì¯â_Pv?Pôkø±f4FGL J1404.4-6159¿í·j‹èt¿Ôq1Ûð+LÀ8!‹P*º¿À9µ+†–‡–@–#BzN@í§m—³?Ä9å>ˆ¦Ø?Ø+G¬fû¸@…ÂL@J?ÿBe"C¡À¿à-Ný¿?¸óºLl•*¿åA1ÃÇj¿ì4œŠâ¿ï«±äéú¿ïäa¾áҘOTHERsppSNR G311.5-00.3?ÆÞf¡ó?Ô8œòøp?êHfXº—ƒ?Ô8œòøp?N煋@Í?¤9tÛGÒ?ï}ˆÃÓ¥ú?¤9tÛGÒ~?±ŠË%qÍo?ªËXð¾ys?íΦ›QÆR?ªËXð¾yr?LÞT¼C??Í4Dª0ý?ïøÈjÐï;??Í4Dª0þ4FGL J1406.6-6523¿íúŸpÖ(cÀ
IJFu/WÀ:;Öç‡À;‰5
þÆD@؆V›Ã@,ò;ò–?Ǿw‰ú?L? ƒy`'æi?܉±¤Ó3™@7~'«cœ¿ë; !³ƒû?̤ç«ud0¿é"kaøÃv¿ä¬åÁX¨¿á§@¡/å÷¿ç~Ò£¦bÖOTHERunk1RXS J140629.8-652251?ïT^ëpÈ?•ô½D
Œw?•t"'ÿG	?•ô½D
Œw?ï׍óÉèÊ? ¼ô,8?t9šù? ¼ô,8?í'È"S¶?¤™¸/¨À±?³é¿óebP?¤™¸/¨À°?ïWÇl»:™?"ï¢îzí?•h˜¬à?"ï¢îzí4FGL J1420.3-6046e?ꝁº‹Þ?ÎÆŠÖ8À8ÄëVûÀ9CQÀ¼ô@$ýýÇ@œ?ÿºjyñ]¦?x´u4ß5¿Ž€ÚZÿÕä?áÉD6¶Ë@
1iEhêпÁ<õ(áu¦?ÏëIúõÕ¿æž¾°nÈ¿åæŒÇ#? ¿éQ%Â1hX¿¦ÀPë!OTHERPWN3FGL J1420.0-6048HESS J1420-607?æb#Í-m?Íá0	1?Ó;¸e¥)?Íá0	1?ì€moJÓ?Î]ÌşD?»ü"‡%©m?Î]ÌşD?åt¹AuŽ?µ+IÉ[?Ս}ñã?µ+IÉ[?ì^We¨—?¼Ѻ{?½ýDÒ»I?¼Ѻ{4FGL J1423.3-5655?Ý:Fþ¦µ@
Þ軶$À9ËýíאÀ;€Px@Â.jÑ@´€Ǒ?Ô((}¢˜?á°:Zná_@	3ä%®æ2@9q‡VËê?ï¯oYT/,¿ÞÀ£ô'b¿ê_$º|¿îÚ®/ªè¿ïâô˜VN?ÒÐXþý—OTHERsppSNR G315.1+02.7?íWJƹYü?À›ö/]?µE©Ê50?À›ö/]?֓,œ³®Ž?ӓBR*ºE?ä¶i±¦(¹?ӓBR*ºE?á£@…nîO?·—ï1ñ;?ܹ~õ"#a?·—ï1ñ;?Åò¡9gu?°ZP+\¬?ê¿CW±¦#?°ZP+\¬4FGL J1433.5-5457¿ïÿ÷€tX@ @¿ã°>À9â2²Ú³?À;šÙ¯3^Ò@)áҏi@5%£þwj?Æ©›o\¯?Ög^~:˜'@Pu-©†w?úX×d«PP?ÀÆtÙpÊ¿ÊýpÄ
`'¿çÇ}³^g¿åWl˜¯ŽÎ¿ëi…ÀçÇ¿ïúñ"l'yOTHERunk1RXS J143329.9-545931?È|P_ ç?ºäû×n©?ï€Þ¾ƒ}?ºäû×n¨?¦ÊLµ®Ë?²ÕAÉ¢Ñ?î"_ë4¥?²ÕAÉ¢Ò?ÃΙªÐy?¬Ã®SÇ?ëY•xËá?¬Ã®SÆ?­ˆ?Ùۉ?"%‡?‡Òá?î'|nBG?"%‡?‡Òá4FGL J1435.8-6018?ÊÚrv@­A¿"`Câ'íÀ8†µò•´2À:'s‡Ù~@Wꞙގ@Vžh5s?ÇrªÂ`ã?å.J€¬¸°@÷jrd¡j?þ%J~¬-?êYà[DŸ?˂&¶M.‡¿åŽÓ朂¿ïQ¢£Y6¿ã3*š}£¿ïëÊSuÈÚOTHERsppSNR G315.4-00.3?œ³ý7·ˆ?±³M>çT?ï'`BD?±³M>çT?ŠÆósh$²?¥S^ALu?ï"ä22_n?¥S^ALu?ÉH]h{"?ºó¶÷??é­è¸%á?ºó¶÷??;®'"B?9nÙ¶|Ð?ïüJ-Ç­?9nÙ¶|Ï4FGL J1441.6-5951c¿âà7ÚWڙ?»AV¥O°À9¯ñŸ,ÞÀ;Ld\ ë@î«8}tö@üÂ]Þ?Ñ+L§?ïþ"ƒÕâö@Ù"d¦@Ö m³·¨?ê®=Ë<©Ô¿í'úðÍ¿w%¡'ϱ6¿áY¥-Ã¿ïüwêó(¿ïàzßDH¯OTHERspp3FGL J1441.5-5955cSNR G316.3-00.00?½ð˃??ȅ^Úø?ì]揘?ȅ^Úø?§1·° Z²?¾Ód	¢û?îŒä"ýúU?¾Ód	¢û?˜?V¢Û?°=Üäùß?éð*WÊ?°=Üäùß?ŠAӚ¯Üœ?|8ï·7¦Ü?ï–ø±•@?|8ï·7¦Ü4FGL J1442.2-6005¿â5Msú¿Á4¾x¡&À8pM'iÒ,À:'_lw! @¡…èÜÎ@Èú½ ßß?½Vx¡k8ø?ÒCf;ô!û@‡ÑÜ×@"Üî^B¿ï§vÑîu?靖¿µ¢¿ã'8Â>Sx¿å"°üŒ®¿ìÒÔMʎ.¿çÐV#ùŒOTHERspp2FGL J1441.6-5956SNR G316.3-00.0?¯¿{;yÅ©?·êæëaŸ?îLHc¦?·êæëaŸ?®?H1Yñì?Â÷t:tôm?î|ê`á?Â÷t:tôm?»*ÒDÝ?©;ê,¢Í?욼¿d?©;ê,¢Ì?²HR'6¥å?¤ûÀÿpÒV?í¶õ¯¹+D?¤ûÀÿpÒV4FGL J1443.0-6227e?Ò0,""ØÀ.>ìÀ9})ž^û8À;ŽÿӊV0@$+Ö²ÿœ-?÷ƒM&ú@?¸Õp_c'Ì?»"™T¥HÏ@X¥H#…@@O~JˆºN¿ïü@ø¨ž¿äpaǛ4¤?ïû
˜	v¡?àÑsZj¯¡¿Ê[Ym¿ÆÞ°zՂOTHERSNRRCW 86?ïûÕÀ§ÑQ?Bü@Ž&?@¨ý`º¾J?Bü@Ž&ý?ï€ÍI	z«?´zÇçöƒÝ?Ì­½¡U8?´zÇçöƒÝ?ïhœêR0²?'Ðb÷N:•?'ìbµ¹é´?'Ðb÷N:•?ï§In/Ã\?S9]K?†-¤t(è?S9]L4FGL J1449.4-6026¿î|Š(m…<¿ê]îBhZ\À8ÛM²:zOÀ:dåÏ@"'^±Ž@ºZƒÚ?ӛÍÐeß?ÐÆ÷ µí@ºç"Þ÷r?û…K'Mð¤¿ïÛíÒ?î@œ<âž¿è÷ŸsÎ-ö¿ê^áÂ}=˜¿ìÕl
?ÆhڟsMUOTHERunk1RXS J145023.3-602718?ÕŠˆ7Ê ?ÏnS(š?å}:»ä°?ÏnS(š?Øð¤ÔË?Ô攵Íÿ?ã‡ó­•š|?Ô攵Íÿ?ÔÍ7¶ä†÷?·´•ùØá5?å™d$¼…?·´•ùØá5?¹D¨¨CÃ9?­ð"쾸?ì×jê÷‡™?­ð"쾸4FGL J1453.4-5858¿æPÁHë;?ÐÏ)~(¤åÀ8ö—¤ÌӃÀ:Z‰%®r@åÀb[>ë@"&~ïÊ?Ëç€Ø,§S?¸MŠÞ|ô?ðx×ÒºL˜@ZÌ´ùòJ¿ÙèyÑ}5¶?ÑUÈôÐ÷Õ¿ç¦G'Jˆ¿èʑž£n°¿ê €¾Z‰¿Ëºzå¤_OTHERsppSNR G318.2+00.1?ԛ'æó?ÒÎk…Ã?å²p7†y?ÒÎk…Â?æJ',ºG?Õ¹­¬á'z?Ójû¦‹qÙ?Õ¹­¬á'z?àv–ë˜ä?¿‹ÿ~Ùŏ?ßÓÂ(Î7?¿‹ÿ~Ùŏ?êÔ¦·Ž+ý?±#Z7­C?Ä­e!ÇP?±#Z7­C4FGL J1459.0+7140¿ïú?i,‡c@E
c
'SÀ:*ŒžßS¸À<¿45'²E@"w¡ÍÏ@œSE!rA?´Æ¨à"Xß?²)"ø‹?ö³#ä
Öô@mÆáü3î?ÞKs0yD¿áÁ~_¬bõ¿æ|yÞ=bŒ¿èL÷à 灿ê¯þàÆ(ï¿Ù‡÷%ÛOTHERcss3C 309.1?ïýTÇX¦z?.Ӟ‡ða?5YÅ:Ì3C?.Ӟ‡ða=?ïýQhHoÝ?Nâ| û?5t½¼!?Nâ|!?ïÙkÑ"ü®?xÆJ`ìŀ?sJn©b?xÆJ`ìÅ?ïÿ¤'êm>ûåû"´ôz?ÿ6dŸ°>ûåû"´õ#4FGL J1459.0-5819?Ædྦྷ?߇ø\rœ«À:Qo'TÀ;ü;ëh™@ÄŽ˜‰¤@9&Ÿ¦ùÔ?Öÿyvƒ??ïÛ>w‰ú@
q#ˆY@,©óXý?î@Ôqü™¿ïÿÏX˜GŠ?ïýP 슿äÉ>$'ý¿ïÿü¿ÙŸC?ïÿ•!îZOTHERunkSNR G318.9+00.4	?ÐBX´:Õ?ͼ7‰ñ"?çÞÀS¥â–?ͼ7‰ñ"?àÔÂî=?Øÿ-þ«j¾?ÞVz#…ÿø?Øÿ-þ«j¾?Ù»#"Œè ?¼ªÚwè?ã"n69‹°?¼ªÚwè?ÌDb=˜?Á	é´Ð«	?èû.çyðš?Á	é´Ð«	4FGL J1501.2-6624?ÓäځÀ÷ /µÐ1À:Óúœé°2À</†K<@F6­;7@³©ìiJ?ʈüˆý?²¬¿¼°?ì‰8ž2Z?ÿ<¾U¼u?çåWr­œ†?é:ÂG¸¦¿é6Ä¢–¿åË·Ä'Þ¿R'4wU÷Ù¿ïü« —OTHERunk1RXS J150054.2-662400?ïÎèQžêz?}¼‰:&G?x‹×0ŠÃ3?}¼‰:&G?ïí×"±0?ƒ‡ašB.?bá(ÝNÐ?ƒ‡ašB0?ïNâñC_ƒ?§>?–#¡×"¤?§>?ï{#þw;?'y±Ýt?›Ž@1‹?'y±Ýu4FGL J1503.6-4146?ß)ºâjë@->X¡UPÀ:ôx'Y
]À<_JÚåª@ <','Û@éLz,	?ÉVöœT	?'Ÿk¯j?É,{Éz?ýH=ägF?$_öŠ¶¿èfÊo${
¿rÈÕ`3
]¿çÛêw¿¿àŽn—€¿à`Ý?á—_OTHERspp1FGL J1501.6-4204SNR G327.6+14.6?ï÷pçí?L6)tw€?QÇ0%óL?L6)twu?ïð'Òc°?€'J?M™?^Ü[9òŸ¤?€'J?M™?ïԈ&Vï¸?w¾¯R[?u»ìԈ#±?w¾¯RS?ïS–cÜF?uóoç?‹ëgî–?uóoç4FGL J1508.9-4110¿ä´ MؓÙ@-F§&J¥À:ÝÿTßUfÀ<'…o@*@Kڔáy@ñã݊Š?Ò'™¢ÓÕ?è~è]¡ñ­@¶,ºs-õ@y,¼¡†?ï)'Dé>¿ÒփDm˜4¿à(֞椿í'Í+d2¿ïÿß^IâL?¼ð&n(҇OTHERsppSNR G330.0+15.0?¿jâÕ]ú`?½½s"$'e?죥T@´?½½s"$'e?¼ØK+Ò?Æ¢ÑÁ‡J•?ìždöš…?Æ¢ÑÁ‡J•?ƂvXá?¬‹žÀ¡™?ê_|"i؇?¬‹žÀ¡˜?±N˜×àJ?š•>ØLÿ¡?íÖ,åýV?š•>ØLÿ¡4FGL J1514.2-5909e?ïÙā,ÿ¿óW"ëïyÀ7§È‡Ã®@À:ä¥Xê|á@!Á»¤[iˆ?ý<96's? ›ªãÔ?s©…ž/Ãw?яãÉén@KûXÑRn¿æVc"3Öǿ䭕X¥´¿åÌeÔp/=¿ÔuÜyh¿ßÍ܁˜¡¿É(èÁõÙ6OTHERPWN3FGL J1514.0-5915eMSH 15-52?ïä#ßR߯?pRòŒéî?kÜ ­ QN?pRòŒéï?îbˆ‡"®»?wù#›?©×wÕQ?wù#›'?쪘×?¬	{%¸U?¿÷j«9G?¬	{%¸U?ì5kunïµ?³Ê$5a?¾T¤Tˆ'W?³Ê$5a4FGL J1518.8+0203¿ç‰ ÝÄd³@G]{á!îÀ:¯c>"¹†À<bã¹x\2@NóÄÞ@è@,¢Ûa»?Ð2&ìS?Ýï!‹k@Û·-[@9È"Ãú@¿ïÿýF\I?ïÿíUÙPi¿à%>þÃj¿çÑt!N¿ëçÇ$_¾¿ïRþª•jOTHERglcNGC 5904?ëï!B¦÷?ºnqÓú?ÀCz÷d(?ºnqÓú?썙cÿ•?ĜÈCÖy-?»"4àW?ĜÈCÖy-?æ5ý‰d!?´ómDî?ӔíÝ7½?´ómDî?ál4Þùc?¸Óú)-kY?Ý&ý–B
9?¸Óú)-kY4FGL J1528.4-6729¿ïúé¼Á­À"X%[À:·ä‡ÔuÀ<qfŠx"f@!
Œ!¶Þú?ü¢î¬ñe3?ÈZKæ]l˜?¿ä†Ò… ?ú0– ÀÕH?ö¿Ê"xzæ?ïþŽø›ˆ¿ÝLr^í T¿ãÜT)M¿Ñ¹Á¢w8ǿݬðäY0s¿á$I@:ؙOTHERunk1RXS J152815.0-673003?ïüo)c?Boµs•?<†·Äç¿'?BoµsŒ?ï@ö—ÁU7?­°$¦{5?—á-ÕY?­°$¦{4?ï˸Éàji?z4˜ÀÊüz?z#›ÊË'?z4˜ÀÊüu?쐶}•èL?Ÿå\ˆ…Aì?»zLP½§?Ÿå\ˆ…Aì4FGL J1533.9-5712e¿ïÿY:6¿ïÿ"ÞïÀ:°ßé	CvÀ;s­íät‰@(ŽÂ¦]¨?òUav<??ÕÂZµX<?´–ÜO÷?â	>m#
?ô´ù[öö¿ïÜb¦-¿ílÚ>$}ä?픁+äŠY?ï÷ÂCÜΣ¿ä*X-¾,?Æ%{º‹©OTHERSNRHESS J1534-571?ïþ
Ñqrô?4ÂՂ¿?/RèèйÕ?4ÂՂ±?íeDŽ?ʟ…–i©?´ÑÃß÷ïy?ʟ…–i©?îMÓOØ°?Ÿ<úùý'Y?«'"Ëtö?Ÿ<úùý'Z?í7ÖȸJW?¸õ¤>¬6?¶AIº=­F?¸õ¤>¬64FGL J1534.7+2331?à¬u|…v@J‰,à2ÛÀ:rÚ:s™UÀ<t¥µ0Ï@£àE$¢L@YÚakU?¾/$…ÆS¿ƒ@f«
gû?ÁÃì¾Ú›Â@y͸/0ð?™t6!"èD¿åaþÝÁ׿ä]`='l¿æ·a*½Bì¿èÀ0§g¸v¿³XƒàÛޟOTHERsbgArp 220?ïç2˜²áÙ?aœ²ï˸ì?hÍgM'X?aœ²ï˸î?ïýq«¨'?Mb$ˆ•N?4wJ¢»p9?Mb$ˆ•B?ïÞs¿j'=?v•üƒôñ?pÆ J·a¡?v•üƒôñ?ïð·'
Oã?JôW6ÆåI?^Ûå`9´?JôW6ÆåL4FGL J1544.5-1126¿ØÙ'mi\@@9&A³À9=ì0?bìÀ;ÈRÆvq@âd¬'ä@5†S€?µaL̆Ç?ͽyȘá@ºx)‰‡?ú¡®÷Š?ïÞðáT[¿Úiþ Õ®¿å®í¾´Ü¿êy…'ͼ¿êlH"ș¿ïɞs`JOTHERlmb3FGL J1544.6-11251RXS J154439.4-112820?¬Ö5}Nã˜?²bÔÑ¥¾?î2œ¨+Æ?²bÔÑ¥¾?¤‹'÷TšJ?±ÑWÕ.×?î·M€Š¶Z?±ÑWÕ.×?ÓjXÚÌ?³¸±çZK?æJôqS'›?³¸±çZJ?¦ÔL§ñ?'̝$Ç??5†!?'̝$Æ4FGL J1545.0-6642?§t[ä¾J7À"ÃH² yÀ:L÷z€ÏÀ<Kµëæ@"!N"b£
?úÅva†,Õ?¾dZGŸ&?™p1ãŸCŸ?Ü˞":ê?ýà¸L7;+?ïöD_«aB¿ìáT™4¿áW'ÏQâK¿ÕHd]L·>¿ÃLu9_¿Øõ…ÞPضOTHERunk3FGL J1545.0-66411RXS J154458.3-664153?ïüÂx"ó ?2-¾&Ý?9ì;`bÿ?2-¾&?ïü¬¨¸?U'ý£åf?:š¼Ú:"?U'ý£åf?ï4n?göLŽˆ†?aKbˑñ¯?göLŽˆ?ï¹Nwp!ü?pU¥ê7&ì?¬b#÷?pU¥ê7&ì4FGL J1547.6-6601?ä!w
JåÄÀ"ì·M߇À:¤W‰SÑ8À<òÙ¦Ïã@k\æàÊ0@¥2.?Ézô'äs²?±óy^æ•K?é—tü+@áZº5Æ`¿ì"Ö@éÕ?ï÷_²íþv¿í°Ú'ÿ#¿Ô)ªžNµ¿ïþ;âÐ?ïÚÑrMû6OTHERunk1RXS J154730.5-655754?ïã¸ä>á!?sŸ ¼ë—è?lGÁßI?sŸ ¼ë—ç?ïÍ`|=@n?•Ü²K+s÷?yOÁá_É3?•Ü²K+s÷?î"àOUj?š¡t¬?§±û
©^å?š¡t«?ï¼?
¿D¨?w8«†ÃÔI?€ð=P.Õ©?w8«†ÃÔK4FGL J1552.4-5612e?ë͏¢dÈE¿ûöŸ™ÛÀ9Ü'³£0À:úZiØá®@!8X"UëD?ý¹á7½Üo?Á=
w}:?ÅÀ=\×ÇR@º.šG>ƒ?ó/ëb^?ïÿÔač¿ïèë Í?ï1}ñf®¿ÚTÁÔiy¿à&ǟ¼Hp¿æÞ'h#ÕÈOTHERPWN1FGL J1552.4-5609MSH 15-56?À˜,Ñ?¥žâ}9!?¤Çóö}2å?¥žâ}9!?Ù­P×
õé?×ä Kï?ã)W"z…?×ä Kï?èœå§ïÛH?³Y`3?͌i`@'ß?³Y`3?Äã‡NH8?¸8߶•š?êÇ,mñý?¸8߶•š4FGL J1552.9-5607e?ícýádQ¿ûÃ"›5{À7ª·Üz¿ºÀ:RŽ¨¤ÏX@ –=^…F{@¿Å¥'¡?«`Þ"J?µ(™QJJ|@È7 €=¨?ôý>!MØ{¿ä©»Þh?ïÿ—Ôú¿âJq=Yý¢¿ÞF™!N¯;¿äÒ,ó~~¿ßŸ[O7OTHERSNR3FGL J1552.9-5610MSH 15-56?Üä†ïº?Ò¾¿ãÊÙ?áð<ˆu¢?Ò¾¿ãÊÙ?™wòƒ]œ?³;†¼¶{?ï4@oÓå?³;†¼¶{?㪳K­b?¹Â*tsÚ®?Ø«™h¥;?¹Â*tsÚ®?þî"‹S-?yTÓ¹ˍ?ï¸GuÒ´?yTÓ¹ˌ4FGL J1556.0-4713?é™Mâ'9>@EUÅ.rÚÀ9F"'AiÀ;.…bªð@Èӌ.¡ÿ@K¼±Ì–F?¼ueáÙ?™:†¨j?܁M½£7?ä;CÖw#+?ïÿý{ÁA~¿á[?÷fÔJ¿ëwpåEi—¿èVÇ¡Р¿àãÕÈc¿Ô‡^ƒ˜üOTHERunk1RXS J155608.6-471529?ï¹lK)?¬+ìjƕ0?¤þ-5¼y?¬+ìjƕ/?èÐD€÷?ÓÀŒÂb?b?Ïô¾íü#˜?ÓÀŒÂb?b?í¨üàrƜ?Ÿ0	AÔË?²¸üiË?Ÿ0	AÔÊ?×ç âã3?¹ÿ‡½ý0¡?äoðŽf?¹ÿ‡½ý0¡4FGL J1601.3-5224¿ïL/mõM?ÔÓëd'{ÃÀ7øKZqežÀ9ÀBHyìU@^¾†GW@løÿZ¾'?Ã÷ÁÃuU?ßó†?IÁë@ÖO@¯óx?úŠ9\mT?ïìz|àP¿Ñ¾²m{¿èYüá¨I¿íhåf÷…Þ¿ëf`ۍ¿ïäèaþ¢³OTHERsppSNR G329.7+00.4?á†ÛkQ3?Ú\΢Ñ?ÜóþI)]œ?Ú\΢Ñ?ŠÀóvcCJ?¡–B†£^?ï"ü2&rò?¡–B†£^?Ï!% ©¦s?³®à,¶Ñ?è7¶·Õ–c?³®à,¶Ñ?'®|Í;?I°o‰s™?ïþ…þx3?I°o‰s™4FGL J1615.3-5146e?Ì ®1¯¿å3X ÈÀ7ØÏä¯A¢À:o]Ø"ke@#.zìu†?ú#'ǁ&?²¶""Ý?º ~"¿÷@
\irŠa?÷œŠÂ¼'¹?ëWË-\¿ï";C¢í?ïž%"ôÆç¿Éf8ِT¡¿×æø<g9u¿Í)- Í›OTHERSNR3FGL J1615.3-5146eHESS J1614-518?ê—ôÚ´‡?Ź±ûvžK?Å£ä,•-ä?Ź±ûvžK?̶¬ËÈÕï?Ö¤P¤x¡M?èÒTÍ
ʃ?Ö¤P¤x¡M?åø¦™xê?»Ûˆ¨q‡™?ÕÒ²Í+?»Ûˆ¨q‡™?¼MdZ›iå?µ áLY«?ìvSt¬'Ã?µ áLY«4FGL J1616.2-5054e?阶ÝA¿À©ˆOnÀ6â1_ô\^À9ÎÒÿì´Ê@!®š‡«/™@aED­®ú?¡Ùt~Þ$?'¾#3-K_?á¡_²??ühˆ_?îï«>\²?~c45oV-¿àŽ·ó÷´¿à"pð›¿äÓgÁ¿×‹&ŸÇ±OTHERPWN3FGL J1616.2-5054eHESS J1616-508?Ûp»dç˜â?Ñ@í)?âG¢MŒ3?Ñ@í)?àä±ôM;á?Ú´¥ãH?Þ6œeˆ;?Ú´¥ãH?䀠èºZ?»8ìè)ÁÊ?Öþ¿È.‹L?»8ìè)ÁÊ?Ë#§Áào?Áv•-_G…?é7‡þ¤?Áv•-_G…4FGL J1616.9-2257?åç)"´§}@3|€Ç:¼"À:GOµò–À<	÷´#ì@<r¢ÿ@gy¦µ?ǔf'?Õº´|ª@Ú<÷Ø?üdî—!ð?ï÷n@ÐT¿ät<Ëbj¿ßÔ½|Lן¿ßͺ}¿ÉY¿îZŽâ™¿ïÿÿ)@k*OTHERglc3FGL J1616.8-2300M 80?ÎàÆ';?Ňî7Ð6³?èGÎ|üÛq?Ňî7Ð6´?¸]iƒ­˜?ÄÜg …Š?ìôRϊLý?ÄÜg …Š?ÏéTŽŽ‡?·©-dTà?è¾êÜ\^?·©-dTà?ırEG7L?¥í
ˆ€EË?êÓ£n®2-?¥í
ˆ€EË4FGL J1619.8-6314¿ìÕضNuÀ"‹<æÀ"À;N»"¥íÀ<¤$Ÿòy@!ŠÙb\k'?öhó ¸r?ÖuK[žn?Úû•!ººÑ?ù¢aôçž	@µ'§‡ÃÙ?ïŽ^g"cпíÉ_²¿êsŸ¿£n…?á¹O!P\º¿Ùâ`ûÈ¿âU1U¡ÏOTHERunk1RXS J161946.9-631530?ïö2";Ó¾?W"鎧?SšÙˆX'R?W"鎧?ïýBCu!?V‡¥¬?5íäWÎøF?V‡¥©?LG•P?…›ÉF¶Cw?‡™lî¬?…›ÉF¶C{?ïíŒÀ,Ô#?[
/$>?bs?Ó+ܪ?[
/$<4FGL J1626.1-5904?åÏò›swÀ¢	?Câ®À:Ûõ ¨ìôÀ<ªŒ0$‹@ Xs~@©ñ…é¹m?Ãé§c†¸¿¦±€Á™G?è<ÓÅåR@ïÃåG—ï?ïÓýB¶]õ¿Ü¬3$D­Ú¿ëÓ	\ ¿èw~¶ß%¿Èäß¾%±?–''ᶶ,OTHERunk1RXS J162613.6-590658?ïêÒ‡Å^?s_¼-O±]?e-âx: ï?s_¼-O±]?ïü•P?bL­Á(Ó?;Uï7c[?bL­Á(Ø?ïmZžê^±?‹:³Ù,?'T¬"´)×?‹:³Ù+?ïæÝÿ0Úì?^~>Ø3¡5?i"Ï%?^~>Ø3¡34FGL J1626.9-2431e?×Bׂ@0º{¢7ÍÍÀ8.ΉenðÀ:¾É'•q@ÅÍc ŽU@ÌՀÐtø?°ú*~å8?ºãi`/¯_@šÐ=š•B@oXiM¡t?ï¦qï0¤ã¿ÚðŽ•·¿å,¡^4׿äL-ráõ¿æj#?O§¿ì½¸ƒi¬OTHERSFR3FGL J1626.2-2428crho Ophiuchi?êw\ÐQ{*?ÄBŸ4ý÷&?Æ"Œ¾º[?ÄBŸ4ý÷&?ɧǎRON?ÐRfàïA?é–kl-?ÐRfàïA?êÞ3 A?²Ì6žt?Ǩ‡3}Šü?²Ì6žu?Óâ	»ãfè?®7ÍÃW?æû"LŒ?®7ÍÃW4FGL J1627.6-3852¿ïß[Ö äº@²Y@ãõÞÀ9£.>׬$À;‡A©î{s@•Í`E@¨@ƒ}Îb?Á7úÃ*6µ?Àž}5ês?þ•Âú»óa@8þ'¢?ïþ0O‹Y?½ï¦–'7þ¿äAç`ÌÉr¿åYg°ã¿è›lØpnþ¿ßgÍÚmOTHERglcNGC 6139?ìb€‰ds?¾šf€¤Î?¼ëÿC´Ül?¾šf€¤Î?í™YÃhË?À ËQ†gç?³51ç\¹¬?À ËQ†gç?ëEàۖ¸Â?³á
/Ò?Âè|'¥ù?³á
/Ò?ë¶ãÔMü?¤3¾.3N?Á$p®ËÀ?¤3¾.3N4FGL J1628.2-4848c¿ãa(˜É'¿§¦{ªEÀ8ɦ¤D‡À:>žm=ðü@7RÅʤÿ@±y|ßý?ʦE9'ô?Ûß°i¿·;@'mŸ?ËÈ?ø2·bWc¿ïM:'£?ï­¨z-¿ÃœÏÄxëN¿étæX¿î¦\?ñÝ}¿áì!%êuOTHERspp3FGL J1628.9-4852SNR G335.2+00.1*?{Cz.£Í?"‹4Bm{I?ïÉyñ¢¸?"‹4Bm{H?îyt¾Ô`?¡{‰JTéi?ïˆF-®?¡{‰JTéi?¢šGÍT7¾?'Xð݁?îÖ[ƒ*¼"?'XðÝ?i‹S(Z?Y`[?~ð©?ïæét¬×¥?Y`[?~ð©4FGL J1630.2-4347?ïc–Hە1@	ƒÏ:eVœÀ9ÓT&ÈÁ¥À:ý¿;ÒE@ )f*×D@«Ænäº?À8ò9î¹1¿²ÉÖù "?óu­+FÕ§?þZ¿êU?ïÿu+%G¸¿èZ&–m¿êzÿzŸ¿éŽ!€Ù.Z¿ïá0œýç?ï"Ic `ÉOTHERunk3FGL J1630.3-43461RXS J163023.2-434804?ïJsîî?¡¾HüwÆD?–¿±'=Be?¡¾HüwÆD?ë¶Â'äu?Ì¿zN®t?Á$÷`oæ1?Ì¿zN®t?ëâ
¹D7y?§3:쪈'?ÀwÕï"?§3:쪈'?ëUÔ¦;‡}?³ôYçl°N?¨­gâ	?³ôYçl°N4FGL J1631.6-4756e¿ïÝ@àV,?Å>ÜIA'rÀ8;i÷ë^ˆÀ:,žh5s@#‡QàG}î?ü°œ!3?³¬
åpݎ¿›äÚ5+¨? ®¡>@c#ÃԀ ?ïÍÐmk=f¿ïý·áXJ?ïh_/:€/¿â;&a"˜Ï¿Ü³±ÇP·¿Ã•Ýað_úOTHERpwn3FGL J1633.0-4746eHESS J1632-478?í)DQu¦ü?½o¦"f®?¶µÝtRÈ$?½o¦"f®?îuÿÙR¯ž?Ã¥hAû?¨ jÕ?Ã¥hAû?çÌ/C¶ÜÇ?µ¹¼š<P?Ðg¡x'Fs?µ¹¼š<P?í=ò8Š?±¤É,üˆ‹?¶n?Ó¯ž?±¤É,üˆ‹4FGL J1633.0-4746e¿íÓqlOz¯?½Ü—Æ܉À6 þÊuÚxÀ8öÇÿ²|@ ìÒ1æ'@éÓHæ#?¥Ž
¢ÎÕ?®ôßô5¶@'Óh@bëà8du?Ü`àjcv?í¸Dµ;¶¿â_{l‡é¿â£-ab§¿äÜ(ŸÜSÓ¿âù ÀTnOTHERspp3FGL J1633.0-4746eHESS J1632-478?Ëqë5¦*†?Ω9ý¾Ý"?é#…2–u^?Ω9ý¾Ýƒ?´<ŒZ?̘ޕ¶ÖÏ?í|8|®t°?̘ޕ¶ÖÐ?äÁãöñª?¸0fÔî&Ì?×è|8¬?¸0fÔî&Ì?˜e-*õM?–=ad
Ž?ï<֖¨U˜?–=ad
Ž4FGL J1636.3-4731e¿ã8äëxÆ¥¿¿t Ù¬"À7:¯ÿ6¬À9b>G]@ …†× @t[¡çEõ?¬û&Qxm¥?»%A>IøÙ@Û]9—?ÿ=lP‹3?êv?ø="ß¿×Á±[Xp¿å9‡
Jݿ䧤WÚ¿æç: ã$}¿é
ŠA·ÛNOTHERSNR3FGL J1636.2-4734SNR G337.0-00.1?¾Y.¤uaß?Å{"ƒ@b'?ì4Ú+qSÅ?Å{"ƒ@b'?…¼èeFÅ?'ï¬zjÄ?ï«Ý^jå?'ï¬zjÄ?ÝÝÇMx?º·Œ# ?á|ÙC¸?º·Œ# ?pe"?ç¶:?côœÁw?ïß4÷€0"?côœÁw4FGL J1638.5-4657c?£õ+­ÎÔ¿™¬.FºN›À7´Ñk—ÿÀ9*OTÑél@ ¹ñ¨ÏB@H½Þó?þ?½¨K
DŒ!?ËE‹:_e@ŸwÞ]îÉ@^ìJìbi?îelZþ¿ä(05Qñd¿âý™ô2l¿æRɛ¿ä‡¿ê²á~µ'ž¿ïÕ)ÝÉõ,OTHERspp3FGL J1638.6-4654SNR G337.8-00.1 ?ŒD´Á|?¬XzÊç¹­?ïÂí,ú?¬XzÊç¹­?™VOÕû'?°Ó5wp^?ï5MP#t?°Ó5wp^?µÍBl±›?¦§>ŸðH?íFW²i̞?¦§>ŸðG?<
2?tðªlŽ…l?ï»óµ‹Ë?tðªlŽ…l4FGL J1640.6-4632?áy'ËðÅ'¿•aÛížvÀ82]œ"IÀ:n­2ӑã@#L¥)DÇÛ?ým  ôØ?±š!(ïl?˜Aä&Ìn?àïJÀîr9@	'™oþ?澖stkã?äK'Iñ»š¿àsuã±ë ¿Þ_ÂWÿ¿áLʳíض¿½VtUè>îOTHERspp3FGL J1640.4-4634cSNR G338.3-0.0?ç†#QÔoé?Ëü±RbÃô?Ðó¹\W ,?Ëü±RbÃô?ê5ð·Å?Ò+»Ÿù²?ŋ(=#"ò?Ò+»Ÿù²?æw¬Ã¢Ï?¿ø^à\¢?Óñ¦xºa?¿ø^à\£?ç>æ#'G?ÂJpœ\Áê?Ñق3¸Ûs?ÂJpœ\Áê4FGL J1641.0-4619?æ *ïT?´J b5ª1À7rÀCQŽhÀ9hÞZ"Ê@Œ‰G.=@•&§3¶?±B€Ùfè?Ã%>¨Ý.o@¾Oá¿£@ø»h {?ïþ/°Ç³ˆ¿á°"Ýz™ú¿âžÝ¦8äM¿æ…~†T¿êDûbÓ¿ç|VÈc±€OTHERspp3FGL J1641.1-4619cSNR G338.5+00.1?²³Òã¯?ÀV}Yò?í©…£ŠÝ?ÀV}Yò?˜ïôÂ0®?°x®cò ?ï8€Yî¢?°x®cò?ÒÂҟ–ß?¶ÈôT÷)ª?æžô°4?¶ÈôT÷)ª?wËa±–b?i§†‹#§??ïÐiÛ<œÓ?i§†‹#§?4FGL J1641.3-5945¿´l¥Š«3ûÀ!›ÿCAžÀ:Jœúw*À<ëoOC4@UbPW0h@úp#~ŠJ?½¹¾'B?o3§ƒYi½?¯)9£P@I¤µ¬t¾?ŤĚúÝ¿æoû:ža¿ã@Ï_~¿åÐx=~e·¿ãJwB+ɇ¿ÉLáłU°OTHERunk1RXS J164117.0-594647?ïëÈÚ-šË?^øšTć`?d7%Òe5ú?^øšTć`?ïþ¿ô'jü?Dê=¤8²?$¶ÙPFš?Dê=¤8²?ïÚ\)Ð?u²ég"^£?rðQëöï?u²ég"^?ïîÔÕâÓ§?Mß<ip?a+*,YW?Mß<ic4FGL J1642.1-5428e?벲у›5À¸ñ.ñÀ8ãíóŽ¶À;5@qà,@"¸	ò=@÷`¤……æ?ÂApã—êm?ʳ<'è'F?ýÌ–›¸X@cbezÙ?ïÂä¾®&¿½ûå~ŸmC¿á𯕄a#¿éikž´‹¿à
Ýað`¿Æcê
J[ÄOTHERspp3FGL J1645.9-5420SNR G332.5-05.6?ë©Ü~D¬?½O¡Wk?Á[ŒŽíQ?½O¡Wk?ïc'G±)ø?ª('ôj€?"·	ÚÁ$?ª('ôj€?élÛäŽQÑ?¯ª–î*Ðk?ÊLmƸ¼?¯ª–î*Ðk?ìã1T"ÎÁ?¢õâ	–pÝ?¸æu[a‰ý?¢õâ	–pÝ4FGL J1645.1-3323¿ïÃ%(Åv¦@ÇäÅøÀ:b/‹ÞÅôÀ;ÇŸïôð@Ñ¢'dì¿@Ayaë­c?ij»¤†]?œ2EfUcN?Üq°œj"X@mF/9?ïìáxU¿Ìp~WÉÀ~¿éšÁÀ	¿Ý¾Ùå9*C¿Ük
…?›¿è\v"œ;OTHERunkAT20G J164516-331816?ïÀwnl1?'š¹m€r?øDHÉç›?'š¹m€s?ïúÙÁ?fSŠ¨?GÇϔ˜ý'?fSŠ¨?ï1t1½]?•1ƒóÕY²?™ÑyÝTb?•1ƒóÕY±?ïÓûˆÃÅá?e¾0CL?v;ž-?e¾0CH4FGL J1645.8-4533c?î#ïl7—ῧ.€_ЎèÀ7Г¨¾Ð‹À9zc'ŸÐ@ê¶W?ö@DV;u÷Ô?À`"•N?ÐÈá°´"@àÀ_?úål8br?ìVP%"õ¿Þæ[L
¿åƒÚ_Ý`C¿éÉÇÄ¿ì/_i#¿è™¢¾[oèOTHERunk4U 1642-45$?–KƒIš˜?±¤PÛFV?ïM£å³+ô?±¤PÛFV?Ÿ(W9ªµ?±SVwŸˆY?ïæ½F2«?±SVwŸˆY?¦£úsЉî?™)L|?î•ÀXÂ÷a?™)Lz?[hÁ}ã`?Là•ÈSÏ?ïòKŸ~A?Là•ÈSÏ4FGL J1647.2-0154¿ï÷K@:T;ÄÒ,ˆÀ;üè‹+À=»	h_@ wɉv`Ú?üó÷é±	"?ؕ";ᭅ?ïû³ŸÕý@ÏE™›@¥"ºÔõ¿ïÿÿ" 5•?ïÿò> w?£	1à€fu¿Â"ÏÅЄ<¿î/é¿ïÿ}e†mOTHERglcNGC 6218?ëœn¤cÄ?¾:³7qáB?ÁŽGnpí?¾:³7qáB?àWR™Ú~?Ö]÷vSY˜?ßQZÌKó?Ö]÷vSY˜?çsƒm÷í7?¶<ª\喲?Ñù$%?¶<ª\喲?Äٔ›
 Ó?°¤·…?êɚÙ<·Ì?°¤·…4FGL J1700.1-4013c?ï™øoÏ?ôãŽ)ùΎÀ9+©EGÍÀ:´Zøt"@Ä=®·8@@›ùÆ*?Ëq†Àyt?àc!m8¿@âÊÿm3	?ÿEÚdåÝÀ?ïÿô!O…ú?Í°:ˆ¥Ö¿àý)áпö¿ë.ª¢ÖY>¿ébߓxî(¿Ýs—ºñƒOTHERunk3FGL J1700.4-4019cNVSS J165941-401121,?µê',šËq?¹k¬Kšþ?íB¯ºl¦'?¹k¬Kšþ?´Ë‰ñ_Iõ?ė+é–$î?ífŽÁÔÂ?ė+é–$î?üŸfûGû?©·ÅP},\?ëØ&A.?©·ÅP},\?––x'³?T܅9!?ïKOoÜ;ê?T܅9!4FGL J1701.0-2617?°W0MFjr@#Q2rC{À:zÝì¯ÁÀ;æiŸ
w@o=O–Á@Ö3Îc¥Â?Äóöû‰#?Ä
‰w¹?üv[ÁǶ
@V^Ä0›ÿ?ï	GÂ6pÕ¿â
Fªß<¿èݘ—;ˆ¿Ö&ˆ_µr=¿é"^úŒN¿çAÀ>ÉêOTHERunkPKS 1657-261?ì%øz·?¼.ܞ|s?¾Ð?¤*Gì?¼.ܞ|s?爫ÓtX?›¿ðÔù}Š?…¹]‹"éü?›¿ðÔù}Š?î
G}¼–?¦sç^·ä?®¿+ˆ$6?¦sç^·ã?îói·Ç?'¼9Ìo3–? Éf$ƒ‰?'¼9Ìo3—4FGL J1701.2-3006¿Ã+]»¶a@Jì$·oÀ8©2ëƍÀ;"'>E@V.?ÿà2Š–ÇW?°1§—ß]?؅»@]h;@&ÇH!Äv?ü^ÖDoƌ?ïþFA'×5¿ÓP&žzT¿ÝBã_5o£¿ä''wcå¿îɨ G³ž¿ïÿuᮆ;OTHERglc3FGL J1701.2-3006M 62?kÕ%xo+X?e¹ZÃ#7?ïä*ڇÕ?e¹ZÃ#7?q~m?˜¡›Xã
C?ïÝý×ÝÖ?˜¡›Xã
D?Š=™íS?}ÚÍÅçw¦?ï—	›´J´?}ÚÍÅçw¸>þOâžmu¢>ö
4là•Ë?ïÿÃ`:Ã%>ö
4là•Ê4FGL J1704.1-4140?å<Š+·ØÚ¿Æ᳤1ÎÀ8à8¦À:æ5SŸ@ lZ$c·Š@<å;X›£@ÏÓ¥."R?à/SàQäÏ@îÀrKv÷?ý'Êß·¶?ïöÉ™"{¿ãïD[y£Z¿âµj¿'{¿âŸp"§Êµ¿é¹ñÞ&Ò¿ïÿ2z¦KOTHERsppSNR G344.7-00.1?¶Ìsú·Òì?¾FnDµÕß?í&q€©¢?¾FnDµÕß?Éÿ–mæ?Ò±-=œE?é€x$Ÿ‡?Ò±-=œE?Ñ?œ¥8Ç?³Îž‰dË?ç`1­yã?³Îž‰dË?½È]ÿsïÒ?ÃÀ‡Œ"½¾?ìFô@'?ÃÀ‡Œ"½¾4FGL J1705.7-4124?ìäۖ-4¾¿ÑA…±ZÀ8q=†ÅÀ:ÅÒ݈@NQŒÂ@]lÝxì{?ÇñPå ®6?ˤK¤C@Ç@ˆ…ZGt3?û½-Dܨã?ï­tw¡!M¿Íœñ½Ç÷%¿åÈ
L4¿å@@aïß!¿èê'Wގ¿ïù+àŠðOTHERsnr3FGL J1705.5-4128cSNR G344.7-00.1?ùt¹«Fw?¥"Š ³\?ï4Z2¥Í?¥"Š ³\?³?Š¦í—o?ÁÅÿ#t˜I?혫"M?ÁÅÿ#t˜I?Ä
ûÜ"hÇ?®%† å´?êü÷eÎ?®%† å´?¡€€Ô'`?ˁÕã?îç÷ò½Ê?ˁÕã4FGL J1708.6-4312?ƒ'2¢9r¿ü4 HtãØÀ9¥tæXÀ;æñ;A@'2]jÔ@N¿ö$µ?ÍI>7s3Ô?Þ8ÞîãM@YДØ@°{/Ì ?îÅ&æÖ«¿ÚWq S²…¿àºëÄØí¿ãÂ!­Ï±"¿ïVNád‰l¿ïT?‡ÕK÷OTHERunk1RXS J170848.0-431418?œ>´'…Ï.? Öø–'Rì?ï
[ëц? Öø–'Rì?ЧÈ4%ž?ѐ"\¤¶?ç¬åív°?ѐ"\¤¶?µ¾6\†%š?¥Õ'2ƒZ?íH94o;L?¥Õ'2ƒY?Á(5‡ô?¢!¡>Â?ëµò¸ž>C?¢!¡>Â4FGL J1710.9-5247¿î`{K‹'Àï•·UlÀ9þ¹®âÖúÀ;'óá
Ì@N0Üêù@ÞÏŒ0û?ϝ^ mÿ?ÖÔìԍ@ð¨ß‡ºt?ó?ƒ3є?ïÇ:"ÀÅ?Øá=\¬Ô4¿å0†yÇ¿í8⟜é¿ïÿú Âî'?ïÿjÿR[OTHERunk1RXS J171043.7-530019?ë–=ƒ?ÃJ¢x"˜?Á§ƒÁóì?ÃJ¢x"˜?ßø3<òc?ÖI7+ÞF?àæaøÎ?ÖI7+ÞF?àN`韨m?´°7Í3±ú?ßc>,À¯%?´°7Í3±û?·)l.eU?¦¶ô~V¥Œ?íÒz3U\?¦¶ô~V¥Œ4FGL J1711.6-3407?ïo+!Š±@	"Äv£ËÀ9Ÿ6'Ú9À;$É:q@vŽôÏö"@¦NÜ%´?É;Û7ôŽ?ÉxրÂ-@¯~Þ,q@ö™ŸxÖ«?ìÚʆ¡oQ?îÝIúÑÿãÜÀ•†åb¿è`´á¼©¿é/Q/|¿á׊`@²xOTHERunkNVSS J171151-340701	?Ôß#d(M?ËÚ½Œ£ð?ånMÿëÚ?ËÚ½Œ£ð?ÜzÓ넲(?Ó8"í€Íb?á–
=¦ì?Ó8"í€Íb?ßPŽ~Ú'b?½û;â ?àW¸À'ìO?½û;â¡?Ù"άÎ#?»Ø,–Ÿ?ãs½˜©˜ð?»Ø,–Ÿ4FGL J1712.5-4642¿å^kòD"À'^!ôGÀ9˜ð¹À;)Y•Œ@°ìaŒ@ƒxÅä?È¥©GÎ÷?Ü'q~Gƒ¢@óg†!Ñ@¢"¾"y¿×|z"«uå¿å}IÔ+¿çá~o¿é€kà£Ä@¿î""¼ÃjM¿íú¾z$OTHERsppSNR G343.0-06.0?³b°["Ã#?µ'äåü"?퓩ôgœ?µ'äåü"?Ø	Š©ŸÔ&?ÓbcÊrù[?ãû:«0í?ÓbcÊrù[?ÏñâöÌ?²ñ×Ö¡Çë?è‡BLúø?²ñ×Ö¡Çë?°+<x§b'?™¬ë"»?íú˜pë°?™¬ë"»4FGL J1713.5-3945e¿ÈÑ@qJ¿Þ@zcÉSÀ7aÿ¨Â,À:fpÍÈu@";@1ôD?ùµ *­R´?¥#Rj†¾?°Ôñ‰o«@aw]?÷Ž²Jj‡]?ﶘ]Ywk¿åہ›v¿ÐŸv¼Ï)¿Ñ?áAxñ¿×Ś^:á¿Ô…·eOTHERSNR3FGL J1713.5-3945eRX J1713.7-3946?æzã^u²:?ËË3±÷D?Ó
9C›?ËË3±÷D?È©j§'¼H?Ôè >X¡?éÕ¥V6ï?Ôè >X¡?æ`øÙ ß?¹‰ëîínô?Óõ>L¾D?¹‰ëîínô?¾¸Ç•
?¯€TG®RÒ?ì.^èç
^?¯€TG®RÒ4FGL J1714.1-3811¿ï÷&¡Œº3?×5Œ	À8ÃÌõçxJÀ:ºæç*F%@"/ÊF_µÈ?ÿ %9um?»"Ci6Or?ªé^ºS+?ñ+E"ˆ¡@}:«w'‰¿£™1"́þ?ì¦a
¶ø¿Ðþ<[zû¿ÝNjܗÆ¿ß/Ÿ•\7¿ÝR€*‡¾OTHERsnrSNR G348.7+00.3?홪ÊÎlj?²†9™»%Ã?³2©©‰Ã¼?²†9™»%Ã?擥Ó¾ñ?֏˜øÁ"&?ÒصX'?֏˜øÁ"&?é›
ŽG"?¹'Kdðù?ɓŸÕÆáò?¹'Kdðû?æ¾Lá¬hs?¿%›í7S?҃f<§/?¿%›í7R4FGL J1714.2-2928¿æȜ\£Åè@¥w–9'ÉÀ:Lp–À;"7À`­À@"ò}
—´@
ˆ~¿"À?Ìéÿb¡4î?Ù
°Â«
Û@—'YY7ª@µ2Ò:J¿ï?Wc"$?ïÿ×á¨Ññ¿ä¸¯©¦W¿âá4bÞª¿îa*ÝyBa¿ïþ]~
qôOTHERglcNGC 6304?ÛÉ0þÁqÖ?˽"9~6?âg€ŸG?˽"9~6?Û¾ý]7¿x?Ô6¤õç¿?⠁Qd D?Ô6¤õç¿?×L˧‹®?¹ðch{uå?äYóš,:)?¹ðch{uå?áQaWHl?¼®Ï°Áʐ?Ý]=Qo'Þ?¼®Ï°Áʐ4FGL J1715.3-3832¿ïp3X~C!¿ªl^Íë±À8ƒ~Ù#ó$À9¤*ëf@£#âqŽ@O	zÓõ?Òµf~ºC?Öa¨üãëÍ@!µÇ͉‹@G+ù4ä¿Â?$ÃÍÕ?翞æàtI¿å^*Ýúº¿èYP¤«›¿ë¡›%ŠÔ¿ïê­R´ûOTHERunk1RXS J171538.1-383531?¶{Ô)Þt?œ Zöˆ‹?í0…zÄ1~?œ Zöˆ‹?ª2YÔGm°?¼Û"c:Ý?î\Úb»‰%?¼Û"c:Ý?ÀhA2)?­1Û@à?Ù?ëú%ø/³v?­1Û@à?×?¥ZÃ÷Pÿß?›Ø«‡`?îªSÀŠð?›Ø«‡`4FGL J1715.8-4549¿ïA£61ä§ÀdÜ"«%³À:oÅåÀ;o§ÿê9@ZÉ!œ‡á@^ne8hý?ÓÒo##p?ç%  ß^@u‡CUÀ&?ÿgþÏSd×?ïό/MËe¿×ÛÙ°
g¿×ED'»Ü¿êE€½ªšô¿êm[}Ë¿ê…M²:zOOTHERsppSNR G343.0-06.0?'ñî?»:–?•áùYï?ïppŽ&+?•áùYï?ÍñXqimè?ÐÔ£àÌ,|?胩㥤†?ÐÔ£àÌ,|?¸9«)‰÷ø?¤Ò±‹s¢l?ìøʚÎÁ?¤Ò±‹s¢m?¦D¬Ã?'ôìŸq?îž>ϛµ3?'ôìŸq4FGL J1716.7-2808?âXv\0B@ú&€IRÀ9M'¿°"˜À;'íû½ñ@­ç"^@Ìã"y§Œ?»ÙÁÎ7?×FW}?pÙ@ªTà,%"@ÜðJUd?íay,;È-¿ßÏÔ¿	•«¿ÜYB'uê¿âÿO™›G¿î3eˆ¿ïòüÂ÷ÆOTHERglc3FGL J1716.6-2812NGC 6316?zo‹P'?w
جò!'?ïËÓ!Ðé^?w
جò!'?˜**2ó¹ç?±$vq~Õ'?ï>®®hb0?±$vq~Õ(?¨'nh4þ?žžó'.¤û?îvÙ|¾à?žžó'.¤ø?³Ä£›$?–ցlcj4?í‡oˎœ?–ցlcj44FGL J1716.8+4310?ç¦Røó@Au¥ 8LÀ:¿,;È-+À<€g€AÙ¿@l[…íõ@¥Ÿ<pÊ?Ò Š#¯Ý~?àȶd«{@¤ò®å¨@ñ`°D
¿ìõ¶ÀÆÚ¿Ý c¸6<Ó¿äBej½ãü¿æXh¬'Ãâ¿ïÿ½OG"?ìf³ÞiW]OTHERglcNGC 6341?íqj͝Hd?·uÃl¬üð?´t©"¼Ý?·uÃl¬üï?íQæn£0?Á…îÑì?µw@̊æ?Á…îÑì?è´ïÉ;?±™C¾ÑPf?Í,@ۇß?±™C¾ÑPf?ì!®"‹›?¬©‹T"?¾ò‹[£'y?¬©‹T"4FGL J1718.0-3726¿á#îa¥
?ÄÅąU"ÝÀ7}5¨Xy>À:*ôàM/@ Œáºö·@Ϊ¦1?©šÂÓ=™?¯J+Ú#@¶w¦)ÊÕ?ûѺyãò?îÀ]ÔÏ¿Ø`Sý®(¿ÞÛ¦d-Q¿ãOl-Îo¿åGÞeü^¿ãÿíPÐÓOTHERsnr3FGL J1718.0-3726SNR G349.7+00.2?Èò8þ‹ÄÕ?ÎFΉ>Àî?éÃqÀ]Ë?ÎFΉ>Àî?³wP²nÕ?Æ6¹!ê?íŸ1é²%?Æ6¹!ë?àÃóÆá6Ï?Ázµ‡ê N?Þxr='d?Ázµ‡ê N?°*'øpgð?¡ÝIæäe?íú­Àñó?¡ÝIæäe4FGL J1718.3-4445¿Ì'—)Ä-À]'@.Ä9À9°"6[àÀ:áJß!c'@ …úUq!@ºizíÜè?Ñ3éܨ#?¿«ó¹J¹ã?÷rï
å?ÿ_Ñâ5iÄ¿ÒC¨ý?ï!ÿ¯"B¿ç%ƒ—×ø¿ãV;`~Dÿ¿ëÑ4Û©ßb¿ÛŽã»{ÂOTHERsppSNR G343.0-06.0?ç%°ç[©ó?ÇrògRt?Ñ´ž1H¬?ÇrògRt?鶎•_'?ÏâIŽ?É%Ū÷ª?ÏâIŽ?æmUíCP?¶ˆQ×Ú^?Ó%T%yb?¶ˆQ×Ú^?Þíã$ž?ÀƒÏ Çâ¡?à‰vŽmð1?ÀƒÏ Çâ¡4FGL J1719.2-2943¿×1館BÊ@}¿Î·ˆ˜À9Ú¨ÎÀÂÓÀ;(ÇAr'@ !f'jþÒ@¥BDH.?ÂXIؑ&.?¥Ä`A´*j?Ø»›!."þ?ö"±ší+½¿î¸G¿²2?麗*¿ÂypÚ2»ê¿æhÓ]à…ç¿êèûlˆÍ?кѢŸ|³OTHERsppSNR G356.2+04.5?éü̾?ÀÕ˜lÓ×?ÈÏñ߇?ÀÕ˜lÓ×?ê¼D5îà¢?Ð
H¿ƒã?Åï(D}x?Ð
H¿ƒã?é†vsÚr=?°®§á·r5?Éæ&0–7?°®§á·r5?çcï=Ÿ9?º–Ÿ°%kq?Ñ8!…þÁ?º–Ÿ°%kp4FGL J1719.5-3858c¿ïì;gy¡L¿îýÕôéLÀ96^q¥^ÊÀ:‹™¯i·@€‹Ò† @Õë#Ïèá?Í:†ä‹/t?ÓÄ7Kæ@tËáëB?üû]y,畿ïÔY=ÞÝÆ?ïߘa5O¿âÀŸAú m¿êD
û¿ïú}¢Ã¿în¸å;rOTHERunkNVSS J172006-385734=?Í]GE}úZ?È

"œ¤<?訮. i?È

"œ¤<?ÁºhºK??ÈH¯'uÓ?ë'eÑ{­1?ÈH¯'uÕ?Æ`Ô˜×?³è"7bN?êz'܊ÙÊ?³è"7bM?¥—Ó½²ZC?—Šú½ß%?Ä$Ú\?—Šú½ß%4FGL J1719.7-4500¿ÒM™ƒÌ}0ÀÃkL4"À9°üQõ–À;¥5¯v@H·"ª—C@Ók'/É?ÎÙ6´Þ?Å°"UÕJ?þ*Óé À@#T²^âd¿ËP§!íeŸ?ïüFlÊ¿è2æ§ieõ¿áȬar`Æ¿êv?A´U]¿ïՓWPOTHERsppSNR G343.0-06.0?ÜúdN&»?Ìą±€¿Ö?á'ÍØ잢?Ìą±€¿Õ?é]6©nw?ÏLÒ¤"@?ʋ%ZEŠ&?ÏLÒ¤"@?ã·úr?ºðt¿¥ž—?ؐÅÕÅ?ºðt¿¥ž—?ãr­y xÎ?»5šÝy¥/?Ù¥
¿e?»5šÝy¥/4FGL J1720.2-4757¿Ü"jœ[ÀÀÓI¾óÀ:'˜Ë=À;K§ågÎ@¤àDMâ·@¡/ÅÀi?Þ³ÞY<1?âéà¾ò·@	å'^éšc@ۚÅ都?îÁr'¿ãF¦ã.8"¿êí¦â'Q¿è"s?ã­¿î±CD"o¿ï¤rØœOTHERsppSNR G343.0-06.0?Þ«{5¤žo?Ó`€T1K¶?àªBe-°É?Ó`€T1K¶?à0{Ljm?Óý_âùj?ߟpïó&?Óý_âùj?Û©eZžF?¹Šmj‰õx?â+MRõ0Ý?¹Šmj‰õx?¼0vŸtȉ?§Ôò+©²z?ìyñ,fð?§Ôò+©²z4FGL J1720.6-3706?ƒ³(v^¿°¸XÌtã,À8§?LF)°À:1²þÅm]@>w|ŽEþ@S½Ö.u?ǚÕChài?Ø ê@%@6Vîú??ô–óT Å?énÑnòý¿Ü.®¿²‰¿á½I6ª¶ø¿èÚå>]³º¿ïÿðEwÙU?ØddIU´OTHERunk1FGL J1720.7-3707c1RXS J172051.9-371033?Ÿp'2•
?½Û—€@î?ï{{îkX?½Û—€@î?·"í
?Å?#Ñ,»?í
b]>¾ž?Å?#Ñ,º?¡L
õ+§?"
‹èm Ø?îë? ­E?"
‹èm Õ?_Ÿž:P¥E?Mrâ,"—?ïð00â×®?Mrâ,"—4FGL J1720.6-5144?݁¥å"ûÀ ¹y[5°¼À:¦úX÷À<"hê¥$è@ ²šl'p‡?ý	¨ÛUüŒ?ÐŒ¢:R?ÐÜ¡'N?ÿàjْ­í?ÿøwWû>¥¿Ý¼âÉä:¿ïÿÍ?¹Ss?ïÿþøþ"¿ÂÜËG'	¿ç+ÔÏЍL¿å»¶ŸŽÑOTHERunk1RXS J172032.0-514414?ï×à9D"b?s¥kü˜u"?tã]µÎƒ?s¥kü˜u"?ïí'lC-"?rQj=b?bؓ¼ÒÞ°?rQj=a?îZ,5Ç?œŽ1$bo?¦/ª]<£™?œŽ1$bo?îÛݟI{?'-d¢"†?¢B&hN¾?'-d¢"†4FGL J1720.7-4629¿ï£='¤oFÀºÆü©3kÀ9«;_QŸ/À;蚈¬â@,Z¢7øÀ@
=f?Ò&Mà]£?Ú
™¶õÊó@ýÌI?ü…jpUÊ¿àŸÖ"Ì«??ïø m]Ñl¿ë<7ž|ØC¿ïg6¥®zÒ¿ï¦J'Qž?'rs\e~OTHERsppSNR G343.0-06.0?í7]•U#d?¾^(ifýu?¶EUVäÝ?¾^(ifýt?â'Õc'ø?Õ-ge÷;?ÚÜU8ûÀ?Õ-ge÷;?à×|»Þõ?µƒ/z}þ?ÞQ‰ÞB?µƒ/z}þ?ÃMÐeÂñ?¯u
Œ£6?ë,¹æD?¯u
Œ£64FGL J1721.7-4709¿î‰Gjb»ÀºeÏg±ÀÀ:Ɨÿe¦À;œèÔjP@£©blD@¥ýfȌ?Í喝:ã×?Ò@$]Wt@,^b‹æS?þ-
gbé?åùæuë>¨?×|Š_iòã?ìÁ֙Õ(¼¿æ˱ÿÁ쟿ޒñì7Ì¿ïþŸã_¶IOTHERsppSNR G343.0-06.0?çrÏB݊ ?Æ]'sÄÿ?ÑazDêÁ?Æ]'sÄþ?î%šG^?ÁàÐÒÍͶ?­¦^«z%?ÁàÐÒÍͶ?åûÙÃfýú?³¸b¨Ár?ÔLy2?³¸b¨Ár?çô퍻Šª?ºökpç<?Ð$äˆê¬?ºökpç<4FGL J1722.6-4529¿Ùl3¼I5NÀ…³ž'ÔÀ9¯Ëú>õßÀ;²Lþ
@ÝS­§@ì``'çÏ?À9yþ§?ÔØVB×Àò@'j¡^‰ù@kn|Šj'?ïµïpeé¿ä±¢Íõ¿ß
J 4¨Ô¿ã‡#uP5¿ë©ÿBjß¿ïúêû‹ýOTHERspp3FGL J1722.9-4529SNR G343.0-06.0?±ØÅ?™ÍÄ?²'ºÄ«û?íÄçXÆH?²'ºÄ«ú?Û"iñŠƒ?ÓJBWAŒS?âu5Ë:¾?ÓJBWAŒS?¼/•bXê¼?©½"T¦®@?ìz
S´â¨?©½"T¦®@?Ý>Moµ"?­eU¸Ü{+?á`ÙrÈ%5?­eU¸Ü{*4FGL J1725.1-3408?øÎ"¹?ë2~žºÀ8ß\Q9®wÀ:I‹N};•@N.4ñ¤H@îu5¬?ÉNÚX¦Š?¸Í®ôõ‹?óü8Dêëœ?ü§5Ù«­m?ãØ'>2j¶¿Ú»k{y"¿çRª&¯—2¿åjþ¦Ž ¿ì¶ ¸Ý,¿Ø/EâOTHERunkNVSS J172445-341032?Æ¿¸L6¶?ÈüѪdc?êP?ÑìòS?ÈüѪdc?âޘ(º¶®?ÕÕלœPŠ?ÚBÏ®Š'£?ÕÕלœPŠ?àùÙÚO?¾ew¹…Z?ßè
ÄLKb?¾ew¹…Z?ÝG¤v8t{?¸÷Ò´YxG?á\-ÄãÅÃ?¸÷Ò´YxG4FGL J1726.0-2843?îÝ(ÃçH@
çTm?žÀ9ö·ü[/ÑÀ;Mx2@Äì@ Óc®ün@7‹7GN?Åa°ÊÓù?…³sy8>û?ÆZgª‰+?ü{Ã	ÕkØ?ïNj׆¿âÁž€‰'\¿ç	ýڶſåf:âT¿Ö¯šâÄÜ¿ãyÔ½\OTHERspp3FGL J1725.1-2832SNR G358.0+03.8?ï¨b¥pž?ƒÌ*ësä?…çV£ÛØ£?ƒÌ*ësä?ï)\VY–?µQ£›"eˆ?œšÔu4ÍT?µQ£›"eˆ?îa¨U!­?–›qú?©åz­å&ÿ?–›qú?½¤˜Ð?'ÁHž&G?¤tt%¶rþ?'ÁHž&G4FGL J1727.0-3835¿Þý7{¿ÿóÐFÕÀ9á¿uÌ4÷À;ác\ƪ@ëE	¬§@a/	ØÆÖ?ØY<k?éÇE8ï4×@
ÜT^üå™@'Ö†ßÙ¿ÂXG"©¿Ùn<‰J"¿åî'Z·Ü{¿î‰¢«'¿Ô×Q?ãšÅ¿ïÿs³VBOTHERsppSNR G350.0-02.0?ãÓØ-á5?ÐßðSLÏ?ØXxϤ=–?ÐßðSLÎ?î£*õÞâ?¹=iê©0?¥ÍP¢߁?¹=iê©/?áÊǛùe™?¹›æØC¼¢?ÜjpÈ
4Ï?¹›æØC¼¢?ì*ÕZgN'?¯*p»%9®?¾©U,ŋq?¯*p»%9®4FGL J1727.6-3050¿Ñmk£""A@@€"ÐÀ9¼'xêÍiÀ;<Zݜ'é@/§x#@ŸìÝ
Œ°?Ç~÷?×q,½ùf@	C¦GýÆ@kóā¿ï·âÅ\–?ïøÙ?Ìɝ¿ÄðÂuZõð¿åZOÈl–¿ê} >ÏH¨¿æû¼Ú'.OTHERglcTerzan 2?¬xr"o?«sÂáÛ¨?î8xß¹?«sÂáÛ¨?­‹ÌíB?¹4¢aL?î(C1.ü?¹4¢aL?ʁř'ü?±[Œ)Ë9?é_Ž™ŸzB?±[Œ)Ë9?ÊcÇÅٜ¢?±ìêf5Jä?ég‰˜×?±ìêf5Jä4FGL J1728.0-4606¿ØŒ5˜¥ÐÀ
çO/<À97cf×¥nÀ;-±@óL/Çn@¿Ue""?¶¯ÀøXA?Ò>¨\U†@"q VL=?ø3
ÎʨÛ?ïÿÙ¿y}¿ß$Ěúݿ჆g­Ó¿æ¥ÒWPHî¿î¸Ÿƒ¾f¿ï÷q†U7OTHERspp3FGL J1728.0-4606SNR G343.0-06.0?œEÞ,ñ¤?Ÿ±48 Qã?ï×I˜s?Ÿ±48 Qã?˜èôDÎLA?ä[ùGÜ?ï8¸]ٍž?ä[ùGÛ?ªÚÏSíQÖ?œì²Ï'×?îRS
Á*â?œì²Ï'×?€È"
à…?g35Ágf)?ï¼Ý³Ëì?g35Ágf)4FGL J1729.2-3641c?ï
}–¡"¿ôŸ(NÓ£À8Q•p?-<À:LÁ¬Zg@·
Rê2¹@ríãÉª?¿z—˹&}?Àp£$è@SÍÅ@Ñwò)þ?ïà!sNÑ¿áˆ8õë¿ákz¢]z¿éOJ@ì¿âŒÍ}÷§—¿ë	—"ÆÔeOTHERunk1FGL J1729.1-3641cNVSS J172917-364008$?ÝpŒzqd?Ñx°°èGL?áGú9ÂÇN?Ñx°°èGL?×°ø©AÏ?ÔÄ×Zߥ?ä'ƒ«_|?ÔÄ×Zߥ?Û9P³ñ?C"
 ¦?âtcW¦t?C"
 ¥?ђš
'Q?¹d]¡"£¥?ç6²ózìX?¹d]¡"£¥4FGL J1729.9-2403¿äßÖáß@@]•ÝLwÀ9s†öÿ¦À;)½¥œà@̏›"ï·@ìB 6m?È{™=´?â}
!P² @"‰|ëãé?þéÁ¢w8Ç?ïü×÷£:,¿ÔÌÕUc¿ã¤¡Ý5¿ëÿ‰b"ʨ¿ïõê28ap¿ïù)¢ßÇOTHERunk3FGL J1729.7-24081RXS J173013.1-240234?¨ΐ~¾?ÃÖ¶MK.‹?îø?ÃÖ¶MK.‹?ŒõœÂÈP¬?ªQ=¬h
Ô?ïŒ)ŒôÞ¼?ªQ=¬h
Ô?£,ÌË'›?•ØÉ
P'?îÍ33M†N?•ØÉ
P'?p,ürÁ»?Vs'ÝòÝÒ?ïßŦ}?Vs'ÝòÝÑ4FGL J1730.1-3422¿Ë£ê¸^ÿ¿ÂGUêmFªÀ8¦Žt¢À9šÍÔ3É[@¡Ìzd@½Ofo ¢?ÍØ&ݏg¼?Õëòa±ËÀ@'؈v\?ö¨Z†¬Ø¿Ü«®¤Ã™G?ﬥDȆí¿åހ¾×@Ä¿éclK'µR¿íT¿	•ªø?"Ö9`°*OTHERunkNVSS J173013-342115?Ëf:Ã$¾×?ÑvT[—?é&qO6ÐK?ÑvT[—?¦€W09¨?¶Ý4Í%"?î—÷*Œüe?¶Ý4Í%"?Á_‰"çN?ª&™(`?ë¾hšÆ-?ª&™(`?gµlÀU4?[¨á64ûÉ?ïèJà"?«?[¨á64ûÉ4FGL J1731.2-3234¿îdz«q1?å$Ðd1À8yÃ
0j+À:?–fß2*@`¿ÞQÚ@,€"Þ?¿^•–Ö?ÓhOŸ¥wH@»4¾?ù@w?ïÂ*|«LJ¿Ö"¦%=d¿àã7r]¿ãÕ¡Qô¿Z¿íoJpfši¿ïÿ¸aÛ½+OTHERspp2FGL J1731.6-3234cSNR G355.4+00.7?i{Cxúté?{M'`ÒyÎ?ï愼‡‹?{M'`ÒyÎ?‡•ú쏢Ã?"ƒ¼üE?MÁu?"ƒ¼üE?‰–9ïJj?zõ/
‡ ?B×Ó?zõ/
‡¦?j´dHœ× ?UN~¹u±?ïåK›·c)?UN~¹u±4FGL J1731.7-3445¿²Û\ªwÖù¿ãØJ¯P»À9£££Þ–úÀ:ÍÛÌDÑ@!ö]¥øw @mŸ¸—Œ?ÂxžözÆ¿¦ÉÍÂÐ?é÷3]z"@û»!ԑ?¢·µ8†">?è–._äÂ¿è‰ù¥ôò¿ß''%οêNûæ•Ë¯¿†WýS8OTHERsppSNR G353.6-00.7?çpº""û?Åtꐀ¢=?ÑŠöäØ?Åtꐀ¢=?ëA/å?Ðøèé36?ÁŠûAˤh?Ðøèé36?éø å%£ß?°*8X'€?È|kip…?°*8X'?ìæҜ%s¼?­y¼­³«?¸ÉkÔb?­y¼­³«4FGL J1732.8-3725?ì¯;ìý>¡ÀCÁð`À9eV2;¼oÀ:ìÍ҆J1@"~'¶Ñ@åH©¼ýL?ÑSÇ'q^?ÏmŽä3ñŸ@ˆÚ¶š[@?¯uxýî¿í$Ò°+¬?ïõ9Ó`dÅ¿èê$@ÒA¿ä—™^á6ç¿éÿD^(Õ6¿çÃlfZ§ìOTHERunk1RXS J173250.4-372144	?Òp'í¬?ÉQ•cÌ	@?æÇô6ö‰*?ÉQ•cÌ	@?Üý
'VîW?Óö‹žó¬›?ázìTˆÕ?Óö‹žó¬œ?Õ¨ºô¼Æ!?·f}EˉÄ?å+¢…¡œð?·f}EˉÄ?Ñ+uÙŽE?º®ÎŁq?çjEu¸Ý?º®ÎŁq4FGL J1733.7-4734¿ì )Yü6eÀ@š$À9ô§5jEÀ<Tsõ›@ ÂÄT­×@ÔF=Ñó?´Ÿ&y¿°ÒÖ|#'@Òß5…@h]‡º;?ïûw¾Q4¿àÝe4Ù&¿ë¢=aàDÏ¿¬ø[EöÚ<¿Úìé7fž›¿Ýã_ ÏmçOTHERsnrSNR G343.0-06.0?ïìx½ž–?d[_{ØÄ?c‡Baiìm?d[_{ØÆ?ïíH|!bŒ?‡&!Ì˲S?b·ƒÞt5?‡&!Ì˲S?ï|®=1
^?Ž·Ü¥Cú?j8YÞ´I?Ž·Ü¥Cú?•È·u?zÜðDq1<?žÚÒ"õ?zÜðDq1>4FGL J1735.7-3026?ëJ
†ZÄ?ðZ|MXxgÀ9êCÖ¦À;Ô#£s7/@Ã՟.Y@âñíÅï?ȃ§¿Í
?ïÿ¼¾ŒÃ@ÖþqŠ†×?ö39=cc¿ïø⚔k¿ï|˜6Ã
¬?ïÿ÷fÔJp¿ßhóžó ¡¿îÈ3'˜¿ïÿyýò߆OTHERglcTerzan 1?£bzRžû	?Âdá1¼1–?îÉØZÖP?Âdá1¼1—?{·£Ý£1?¡çƒ»™§ÿ?ïȐ¸D¹ü?¡çƒ»™§þ?Á²>&ú?­›úeÖÐ*?ë pvA]?­›úeÖÐ*?ûM+ÿ??Œà'´vÓ?ïÿ%– ?Œà'´vÔ4FGL J1735.9-3342¿ï´<*:í¿è¼Ý W
ƒÀ:I¡òYNÀ;•ð	÷y@$>ìW¬@?öúReŽÐ?Òõº+àY?¿/øìˆ?昏Bþ'Q@L¨–a«Â¿ÙÝ>‰þq?ìÕ¨]ס'¿ë¶y¿¾ë¿àt¹°V$¿ÚC©blD?¹kt~hLOTHERsppSNR G354.8-00.8?ïÈnpqù+?…ýʊöîë?{ÈÇÇjç?…ýʊöîê?îµ¹‰g?Áwêfò?¤¤giˆj?Áwêfò?í}¼R+!?§Ÿñ£µö?´n¦ø?§Ÿñ£µö?ï	ª¤…ñ'?šËæôî#?žÊ«oAͱ?šËæôî#4FGL J1736.1-2628?áÛ6d!(@Ž)#øÁÀ9Ë~>Ê@+À;!ë¾íç@8Å]F­@"¨~8ë?Ò.!%"?ގÍbÉÎÁ@z?|ÑÔ?ø@ƹã;#¿ïýV½{öñ?ïþ¤ ³¿5¿è3«=°å'¿æÌü¿ïù÷<âß^¿ïö.$ÖyOTHERunk1RXS J173614.4-262806?×ÑT¾u)Ú?Ï|
És3?äU Åk?Ï|
És3?²¾'èM?Âe‡ÖÓï?í¾0/¢÷?Âe‡ÖÓï?Ï·$_«Òç?³&@œ®š?è6èF?³&@œ®š?kt§>óÂ?Š@}å"?ï¤ZÆb?Š@}å"4FGL J1736.2-4443?ïÿtŽ/Àç"~§¥ÌÀ8¶A+Cz©À;›<Õsd|@4ê³èzR@.Oü—•³?®éùOÛ¤?×{z«í¯@%	¼râv@n¦R9³«?ïóÝ£C<¿³3ãu!¿Ü<Î<Ž{®¿åp³[â~æ¿ï ‰bi׊¿ïõ8%á;OTHERglc3FGL J1736.2-4444NGC 6388?ÂWU`ä±?Ó;ÚÂi0[?ëj*§ÆÓ½?Ó;ÚÂi0[?xúZáœ?'Íàó¹Öú?ïÎJ<ÇÌ?'Íàó¹Öú?±'v-æÊ«?¥·ð4-	¹?íÍÑ:C&«?¥·ð4-	¸?=ª^Ç?3)ûÀ¾8?ïü]ê¿}õ?3)ûÀ¾84FGL J1736.4-4052¿ï«îÔI~uÀÔÖ¡aä÷À:PfiÁdºÀ;¿ÎçY@@XÍq7zÁ@²£Üºî?ÈPG@0q¸?·ÀÙú]?ò4Íg&Ç?þ"š™ÉÀ¿à,ƒì‰*·¿âò2ý®A¿íå*ýÌ=?Ó©£Ò؈¿åàÝPþu¿æ!μ'gOTHERunk1RXS J173638.5-405203?ïáhˆ^Sa?l¤Ì'óß?n—w¡¬Ÿ/?l¤Ì'óÝ?ïÞÒv¸¡V?"Ýw¸¡ßµ?p–Ä£¯U	?"Ýw¸¡ßµ?î·&|ÐI¬?šêJbÅb?¤˜2ûeC?šêJbÅa?ï}ëÀÉ<
?ƒ.ÄeÃé'?B‡æØ~®?ƒ.ÄeÃé'4FGL J1737.5-0313¿éit?h\@-§C"º"À:{i³"ÜÀ<7dè·äÞ@ÆUhgG@üó:õŸT?ˬñ»ÅI?âʹaµý}@žŸj"ò'@
Þ4(Q¿æ²®¨õW0?ïȳBb%9¿Ï_Qߛ±w¿éQß@lך¿ïÿY¢Ò1¿ê8PV×OTHERglcNGC 6402?¦gxt¿?¯)/©g³t?~(´?¯)/©g³t?Ç×QÂvÓ?Ì·ޜ°K?ê
+»ObL?Ì·ޜ°L?¬Úc£A¾ß?˜7šAž?î2YÅËä?˜7šAž?ÆvuOh¨…?¨œÄÙF"?êbb¬%ÕÞ?¨œÄÙF"4FGL J1739.6-3155?ËžPztL¿Þp"ýþs
À8¤nM]À:X"@pǎŸj"@	:ß.Ï d@_å Ù(ü?×6þ™Îs@´ebZh+?ÿ
¢ÕØd?ܪ(][Œ¿åAxÀÛý¿ènrÚ/­¿ì,` ÿ"u¿ä}C!½¿ê¿ä§Œ¡c'wOTHERsppSNR G356.3-00.3?Ôq>FpD?Ó´ë&•?åÇ`ܹGÞ?Ó´ë&•?Òp?R#R?Ôçv*öx?æÇàV÷îV?Ôçv*öx?Ð"›rT«Ì?·³ÃuQ?çî²FÕª?·³ÃuQ?´rwnD?ÁK(n?íq±ò.W?ÁK(n4FGL J1740.3-3058c?ì}¿¹[%Ý¿ºÒ¥ÿ®vuÀ7ès¥ê
À9¥€!ùO@š.êÏ@E×_ÍÅñ?Ǿ%ÀÕ?ДΣç{O@çžóu®?ó»›~ñ"?ì.¿eÛüë¿ÓƼýÌÉó¿æT%B|¿èm`öºÜà¿éÆ&Tþ_¿áº­EH­OTHERsnr3FGL J1741.1-3053MSH 17-390?•;íTE?¶8©*kg0?ïV •]×g?¶8©*kg/?¤*'FYà?µÎ"éäý<?î½Wۚo?µÎ"éäý<?´"Ÿ¹¹ˆ‡?¢ÕÙ2!E?ímŒÈÎð?¢ÕÙ2!D?Ti
­3ρ?F"›è!!?ïõËy)f?F"›è!!4FGL J1741.1-5341?Üü«\‹E¨À(¨"1¡À:1ôú€5À;¼K±¯:@n¢ÔUØ$@t£%3–0?ʏ`Fþ?Ä(©båR?ø'›k*ñE@MGva0G¿ÑßrV^±f¿éQK·Žw'¿ä€–ÉÁ0¿ç||Šiü¿í^æ¤h¿ïþÞ&'dOTHERglcNGC 6397?î·Sƒ&°?¨Š-ZßB¿?¤ŠÇÏ
•
?¨Š-ZßB¿?ïF_)[ñü?¦"ÙcEùx?—4ԁÀy?¦"ÙcEùx?ìîÒE Ò?ªH†"¢Ð?¿‰mÒùn?ªH†"¢Ð?í¢'"Ê—e?—ш~ ÒÂ?²ësY«DÕ?—ш~ ÒÂ4FGL J1741.4-3046c?ïrÎmûŸ¿Éú³åË zÀ9MÛ:MÙ¨À:ØZ@ä@[¸b‡Š@Q¬šþ?Ò±–¡]³?èzÎg×®@à‰ï•O?ÿ³'ú;ñ?͇…oëö¿àZ[–(Ì?×4AðeX¿å"†bZ=8¿ê'Ì®š¿ïÿôým~‰OTHERunk3FGL J1741.1-3053NVSS J174122-3047120?–?q¿¥ö?¡¦·ES"?ïNr×ñ?¡¦·ES"?šcQ\QѺ?°µ~âúÒ?ï,åuqs?°µ~âúÒ?¶Ô?/ÍY?£˜d"´?í%xTß?£˜d"´?ˆK(lì?x46Í.U?Óó^L?x46Í.U4FGL J1744.5-2612¿âñH!ð"g?ú«‰†&À9
	A}À:Óeµf~º@©Wn¦Ñ»@'û'½?Á}Žá"¿Ã?¸?YV†J?ù•œdO4ñ@2¯Õ›'Ž¿¶̶Q‹8?ïãšn«¯¿æ÷?ö:.¿åµŽÚù¶¿äÁN·8¿ÜžWn{ޞOTHERunk1RXS J174419.9-261230?ê÷ž̎™?Ŭäù×?Ä!‡œÍş?Ŭäù×?å¹x8'?ÔªÛ»%?ԍãŽúå?ÔªÛ»%?é±ÙL?Â$hÄÊVÄ?Ë¡8›÷žÕ?Â$hÄÊVÄ?ërÃ	Ëp?®ER0	‡?Áú4óØÒC?®ER0	‡4FGL J1745.6-2859¿Îqˆ\À¿£ï›ƒÔ‹]À5–åápÈÀÀ8ïlÒÐ@ "_§ÛPÉ@…+%G¸%?˜…ö¤Œ'É?ÅÄ¿b+]@/
'Ä"Bh?î•‹Â|£¿ÀÎÊ}è
E¿Ú@ "®¿à&cvÇÝz¿åßEuU¿é<ëج¿äç›O|?OTHERspp3FGL J1745.6-2859cGalactic Centre?¡ÜxGÙb?ÅK¶74¡µ?îâ8{'iØ?ÅK¶74¡µ?Kwgÿ¬C_?[WítŽÜ?ïù"&ð?[WítŽÝ?ŏüƒyƒ?³á5ô"?ê¿ß!Ÿ?³á5ôƒ>uw­Òñª>$´}^jÌ?ïÿÿÿTC>$´}^jÍ4FGL J1745.7-2506¿ï¤»='¦Û?ÿn$…ñF)À:,]VlÀ;À9'ÈÅ@'9òj@yÁ­?ÔöíM"‡?'xë¤@ä5À¬-?úϽ<¶ê¿ïþ~üà;?ïý±Ü†~4¿ÆÐîÚ雿ê¸1Ûã@¿ëð`"=µ¿ðOTHERunk1RXS J174535.1-250440?šñ	Õø?§zšÏjzÐ?ï(w±Wçè?§zšÏjzÐ?‹óð!xUL?ž«5º=Ü?ï0?zª?ž«5º=Ü?À*XÊ*ÁC?©ç|úMñ²?ëõiÍuO°?©ç|úMñ³?p]Zn^‰8?^²yê…"k?ïßEK#Bî?^²yê…"l4FGL J1746.2-3342c¿ál×mØßTÀºAå}»À9¬.þñGÀ;ÑÙ|¸@ôÔ$"ï"@Çz³$…?Ð졾×Ñ?¬Mîd;Í?ç+8ÞøÅ@JÏz?ï~E뜛­?˜¢"ŠwE¿ê)æž/*¿äDïž3h¿Ý
Š2‰~¿ßÃ	Õk׿OTHERsppSNR G355.9-02.5!?ï(¿ãã?¢ù˜]dð?šècŸc‹?¢ù˜]dð?ïîÿôåQD?" íï?a®»d?" íñ?죾üi…º?®Â"hÆJù?ºâ³Ò#?®Â"hÆJú?ï`ŸOn°)?ƒ<‰MsÑ!?"ì)úî?ƒ<‰MsÑ!4FGL J1746.4-2852?Š×:À¿½¯+ÀçÖÀ7b·«cÀ9¨ä:§›»@ €$±0d@­ÿYçÒã?¹²Dxªâ?æGa=‡Ÿò@'¡"¬S±?ÿò©ëJ¿ïÿÖ_Æ	?ïÿu–…#¿É"£{Ѹ¿á͚ݼ^@¿ì–à­F¿ëÿfèle"OTHERpwn3FGL J1746.3-2851cPWN G0.13-0.11?¯Æˆ:ìô?Ë{Ì1HÕ?î—ÌQ1?Ë{Ì1HÔ?SZN+KÓ?aÁšm¯L?ïöRØêZt?aÁšm¯L?°,´oV?¡=²î?íúÉ~?¡=²í>‹­UÑ5>‹á¢™,à?ïÿÿ'J¨»>‹á¢™,à4FGL J1748.0-2446¿èg£#¾'?û&òIÀ7C¼¾aÐÀ:ˆ?›÷Aë@H@
²@ú¦Kaþ?¢ô2ÂJò?Ö'½3Q¼@0¹:>À/0?ú¢3'ÒÑ?î°Ý$•¿Ñp*
ag¿Ýù˜kñk¿ä¸–IƒÑ¿í_›¦º¿ëVxHOTHERglc3FGL J1748.0-2447Terzan 5?CËºH'"?7µ€¬ï0?ïûmß?7µ€¬ï0?T\¦ ~îÑ?t¾
8â~?ïõѬ¯Àˆ?t¾
8â~?×*l±èÐ?Y&ÃáÍHo?︣VM8]?Y&ÃáÍH>bÅ*Ö>fIq{%?ïÿÿíï:Ö>fIq{%4FGL J1748.9-2021?½jzhoý@X䓒ïÀ8íÿS1Ö<À:ä	EùßU@§ïŠçÐ@¤ê/´?¸(^ÿûßp?Ò—=í§@=Ÿ¿MˆI@Åì•j
?΀%)ZAj¿ªnSà&ò¿àê:†ä‹¿çt7ª'8¢¿ê_gJ¹¿ê¼2€…Ì]OTHERglc3FGL J1748.9-2021NGC 6440?Sm©P—_/?LiΗê¥?ïöI+W´P?LiΗê¥?‹¹ô©ãb?™"±ÁAm?ï'-[´s?™"±ÁAm?š8'•°Ù˜?•GÂêì§?ï.;sRy3?•GÂêìª?Ÿî™Aƒ¤?:‹€'>?ï(‹5óã?:‹€'>4FGL J1749.5-2747?ÁôÀ:OKh¿Â1²ªŒ°þÀ9yòìòBÀ;gÝkí@Õ±šl(@mZ˜?тl¡"ãø?ïÚø4H‡@~x?'æ?ô‡×¾˜?ï5ø_w´Â¿Ó'óÂÚۃ?åDª¿[Ë¿âÕub'¬¿ì/bCA¿ïþŒ}QdwOTHERsnrSNR G001.4-00.1?Ç™-ïv?±Ø.¡³Ö?ï€á›·HB?±Ø.¡³Ö?"XI‡Gñ? ®ÿ¸r2[?ﮞÙâá¼? ®ÿ¸r2\?³G(½Â?¡¯\,Cµ?íŸzèH?¡¯\,C´?1³žŒ¬?&*âwºe?ïýßɌ?ð?&*âwºd4FGL J1750.3-3702¿¾!ÈnM҅Àäõ8À8êõÚPÀ;RՔ«@&¦ßh±@'~D©}<?³éçdӔ<?ÑçäÀ´e£@AkÛm@ÚԏŽÓÃ?ïÿ6A­?ÍÝ%OšÈ¿ã
œ5ULc¿ç4"䤿ë68Öá"Å¿åȊ³LÉOTHERglc3FGL J1750.2-3704NGC 6441?xѹj¯`%?}â$Ë?)?ïÎ\*¡A?}â$Ë?)?"\¥öÇ$Ó?œì&æ· ?ï]ÐIÆÙ?œì&æ· ?™/Mzk9?'0‹Êní?ï6…—Œ,¦?'0‹Ênï?….y¢…?mme"ÌõÐ?ï«F›•v?mme"ÌõÐ4FGL J1750.4-3023?Ú-Ñ2!í¿ú'Ã^À9÷q'ÒüÀ;hšQO}í@º†è¼í@Q~B%>~?ÒËUhè æ?寡]³9~@lğá§?þxqƒzô=?¬Ç‰£'Q?á¶úc
¿¿òØ`eÇ¿è¦Æ¨Æ]G¿ë7V]Ú¦ª¿ïïwAU	óOTHERunk1RXS J175019.0-302654?¡Ö)ñi)Ý?¨úµs‰?îâ`émb?¨úµs‰?͜t\D¿?ÏՒ@E`?è˜ûbèîÑ?ÏՒ@E`?É1mV<ˆ¥?²Ý9¨ù?鳤ªpÝ×?²Ý9¨ù?³¡$jjL?"ùŸZû×¥?í‹Ûr²¾6?"ùŸZû×¥4FGL J1750.8-3106?ê¬>	÷¥|ÀÊ÷?gÀ:h²qôÀ;®†Ô@o|—@V[~«×Š?ÓTo—4?ìϵIùHV@©ôafLe@Ù –¦¿æE"~°	H?ï‹ÈUnÇ^¿Xøš$W"¿åÇ-»úír¿îÁÛ!yLr¿Ú–Ý&·#îOTHERunk1RXS J175042.7-310312?MÖ¤õëw?©kªPž?ïºÈ¥l(R?©kªPž?»•Næ?Æaï\F?ìV>=ƒ-?Æaï\F?°¬¿ó3-?ñßÀ=FÎ?íêh™Ÿš?ñßÀ=FÌ?žS³±X2X?†-ƒìø#?ï
bbu>n?†-ƒìø#4FGL J1753.2-2848?â9Ž.Œ¿õ¶2ŒDFÀ:^ıuXÀ;RU.‹.@'Ê'š¤‡@8Ã`<€º?×íK<¿N	?賁6ÌDè@
*=DŸ@‹¤íµ¥"?ì€BŠ3ö¿ç)BïhÙ¿Ó•j \×F¿ã«LŸjéÙ¿ïÿ»×²¿ÜŽÂÛ²BÞOTHERunk1RXS J175328.7-285014?²@Üiå"?»aÀ5»-?í·ärÃ[Á?»aÀ5».?×÷»9›4ü?Õ-œù="²?ä"c2e'?Õ-œù="²?ÏÒ,Öý?µùþêmAM?ètøJ@º?µùþêmAM?º‰\f…ÎR?£<^Kp–?ì®Ôs/F5?£<^Kp–4FGL J1754.4-2649¿îCL®Fj›¿ãåjR"À8ôç¸5fÀ:R¦'¦`Q@T\>D^T@(obŽj'?ÊÉÓH<ç?À˜|¹)?ü}[
Ѻ?ö­…¼?ïÿ%¿Ø·¿æo—@G¿æQî¿æµV¿ç¦üX«'À¿ä'/ÿÌÿM¿æQµ4)Ó8OTHERunk1RXS J175501.7-264954?ä_¢%Þu?Ðú(¤>C²?×@»´CÆ?Ðú(¤>C²?ãâθnöm?ÔÍ/?E‰?Ø:b"&?ÔÍ/?Eˆ?àK2«ý"?Àç†"â.?ßõiš¨Ù?Àç†"â.?ËùÃkØ?´84—'R?é8Ÿ%
?´84—'R4FGL J1755.4-2552¿êkHQ¿Ól†á­¯À8>¡%À:"Où<—`@ ,&dä@ÙYæ%cg?Ç2>@­o9?¼Êm!¤W?þKZ;µ¸´@Û´¡ö?ïø׊•ñ¿ÚN`ÐTí¿è#¿dTh¿åÞ$ÿ¿éó`µL~¿Þ¤pMOTHERsnrSNR G003.7-00.2?Ý?[7´ð×?ЯŒ´­ù?á`Rd%‡"?ЯŒ´­ù?çÿ~;>éK?ÔW+<¾µ?Љ'-k?ÔW+<¾µ?á]Ñ"×ö?¼ÙùÖ"ê?ÝD]ºQÔ?¼ÙùÖ"ê?çÆ"
kË?¸b1šå?ÐsúÙë(i?¸b1šä4FGL J1756.1-2516¿×FHi¿;¨¿À;÷ÒßáÀ8U®mf4èÀ:!vjNR@ûHŠˆY«@À	‹û?Ã}˜F³B¸?Û[Ÿ"š‰¯@²¹šû@è*~XËs?ïÿy'3J°¿Õ:–9üÑ¿áôÌÆпëêry\ã¿êDå!ØAö¿ïÿ) 4ÓÇOTHERunkNVSS J175606-251909?ªðȺs?'Ú%ì>C1?ï¹W¬<Ý?'Ú%ì>C1?qñYŒ¨?›#ù]mù?ïŠ8:™Ï®?›#ù]mø?£`à"GS?™–vÈ˲?îÉñýۏ¬?™–vÈ˳?^ގ•V¾'?LêþÈ?ï𐸵T¡?LêþÈ4FGL J1757.7-2337?îJèÙq&?×ó*š}£À8‹
É^çÀ:¡žJÙB@ å[ºà
@ä=F²kø?ÊQù\wÐ?Å*©÷µ®£@Yí{ì
?òe@çPܑ?Ú[©ôÓ?Û&º>ƒ¿è|X@2õ÷¿á×L¸?w¿í¿5դ⣿ÀS±OTHERsppSNR G006.1+00.5?¢ÕeL¥#«?·c¡P"?îÒ©«5­Å?·c¡P"?§–ÈmÃ>?½)Üèá?™#Í?½)Üèâ?Ά°úÁH[?´ˆÑ¡Ð%ô?è^SÁO­é?´ˆÑ¡Ð%ô?'±´1aµ?y'-¬CëÞ?ïµ9/":y?y'-¬CëÞ4FGL J1758.6-2404?ê<°€š¿£.y5}À89Vº øžÀ9þœCc@ äÄ£³xé@×î['ÍÍ?Àa×5†t¤?³sæÐ_~?þ>ɄBð@@ãJ膑ª¿éJ]ò#ž?î"Ó–ëip¿ê¦]¨R¿ÜÑÓñM5¿áçj¨† ¿í×ïunA&OTHERunk3FGL J1758.8-24021RXS J175835.5-240203?Ú!3iF?Ó4ÂaêÔ@?âþ~ofK^?Ó4ÂaêÔ@?Ù´Wc7ûf?×,ȱp›?ã%ÔNdM?×,ȱp›?á†,\E?ÁT5>Œ¼G?Üó§ÝGów?ÁT5>Œ¼G?æ'OÓîº?Àí±ýí0?ÒÛ`X"‹Ã?Àí±ýí04FGL J1759.1-2347c?î\Ÿþ¶%?OÃ%ãÀ8£hQ"1ƒÀ9Ò`8Nûç@ ½}mi
@"ã^߉h?Ô~/%1'Ê?Éèâ'q	@	Ãa@O?þþ¡ì#6¿îˆ¾ªö
?×ÒíbÄp]?ëéšbí5¿æ"¸žÂx`¿è³†_€>¿è-@ªêúµOTHERunk3FGL J1758.8-23461RXS J175851.9-2345110?²Ula"í?Ã#ÅRcé?íµR}3̓?Ã#ÅRcé?§NK±ž…?½§y®x¥?îûDæ?½§y®x¥?Âæ
ŝó?¯Hö3‹ ô?ëFy=N˜ƒ?¯Hö3‹ ô?³šs ™zî?®2#Œ©³Ÿ?팱‹ìУ?®2#Œ©³Ÿ4FGL J1759.5-2312?ïD¡lF-?ˀæYæ¦=À8©¢ò(§À9ÐaŒâÑò@/°NÜ@ÒÇû¬´)?Ò`ÍX
?Ïϧ¹õ@	àÛ'£H?ýI"='Ûà?êo€Á[€¿èìßý+9j¿àõ\"•¬$¿ç÷ÆÀÄ*è¿æOæ'æ¿ïþ'!€-bOTHERunkNVSS J175948-230944?Ù$ñòÇRÞ?Ðë}ìª?ãm‡œV?Ðë}ì©?Ã$tˆ™?ÊñÅ1† þ?ë6Ø¢Ýٜ?ÊñÅ1† ÿ?Ò'J(c?µæ
Ðw2?æìsÚýkÎ?µæ
Ðw2?¨íÉÂ7â?œR»–@€?îq.Cc܁?œR»–@€4FGL J1759.7-2141?F¤Ð
Ô£?á)À8Ïa€M˜9À:ªh_dêe@Àîó[Í@¯…^y2?¼Ž½Gž¥?Ñ!šÄçÑ
@ÛHƒ&Ž@9Çóʲ?ïþ–Ž0Z¿çôÛߏG0¿Ùzßð&¿å2	g‡Î–¿êC@؍J¿íû,áàZHOTHERunk3FGL J1759.6-2141NVSS J175946-214231?¸0x9Ñù?·–5? åæ?ìùðøÅÜ!?·–5? åå?ÁÀ>"…}X?Ì"n­ì…j?ëðw^ ª?Ì"n­ì…j?̉f»vìþ?´Bôš<¸ˆ?èݦQ"DÁ?´Bôš<¸ˆ?ȹè[G¢ð?©'ƒü{&?éхé.D?©'ƒü{&4FGL J1800.7-2355?îõƒhÊí¿×É] í`kÀ8<Rô™špÀ9Øïÿ×¼@!º˜ó¬_š@(@Že‰?Ä6¨2¹°?²ðãB1h?üJë!L?úúŸ³ºC?îT)'°I	¿ã.ôàM/?ë^ÊÆbO€¿çSÿ[•R¿ÞI½ƒƒ­Ÿ¿é['£HoOTHERunk1FGL J1800.5-2359cNVSS J180041-235622?ԛ|üó?Ñ^'¨š?å²yÁ†|?Ñ^'¨š?Ô`ZEވ&?×;³0=3?åÏÒÝ»í?×;³0=3?Ø•$
eÁ?È_ör£È?ãò5múÍ ?È_ör£È?ɀ2c­`?À€E-'?éŸóg?Ô¨?À€E-'4FGL J1801.3-2326e?ïj+ý³¿Ð:ÛGÀ6,l™†NcÀ8³Ïqºû@ »\æzH@B¥–ýÞ?¬¸oâTã ?ÀÁà [R@!,ÁÊ:KU@ºyŽq¿Ò1܆~3ã?ïsR4¿å•"õÎN¿ãÁè"Ïf¿é9Ò9¿âAî¢_ßOTHERSNR3FGL J1801.3-2326eW 28?yx'«¨M?'.Þåô?ïÍܨ¯f?'.Þåó?fÒɤ2°?z#ä×´"Z?ïéí-6[Í?z#ä×´"[?Ö(¦Çø³L?¶2ƒñP?ä묜¦Z?¶2ƒñP?â9ŸuH?©¢Í7q?ïÿXî3œ?©¢Í7q4FGL J1804.7-2144e¿à‹¹ÔÙ¿N¿¸G7÷é=À7d/TbÀ9J®¯«SÖ@#*0oç@UhƓ?«R€o?î?'IR{Å?²?ïÝDêÜ0@Ë<quc.?ï÷Տ-Ú¿ÞY•‹–¢¿ç…=jĚ¿Ø9›aðµà¿áCœRæW¿Ðø3£¡ÂOTHERspp3FGL J1805.6-2136eHESS J1804-216?ã¨ÛKh
?Ñ5ê ðl?Ø®Iiû/ì?Ñ5ê ðl?ãY$¤+?ÙNx î&È?ÙLß··«?ÙNx î&È?åÅkÎYQ?¸›¦}	q?Ôu)þcM_?¸›¦}	r?܊®ôÞ¾?Ç;ŽÓÏĈ?Ẩ… ¸?Ç;ŽÓÏĈ4FGL J1805.6-2136e¿åλê«Ç£¿Êó› ­JÀ7cÿ¥g-6À9A¹d:<<@ Ðyšu·'@žš|îh(?·6=>Nð(?¼¾-]íWB@*{[Àðö@åŠÞÁ?ïûþQ)=¿ï÷" fQï?ï¹ý‡»¢¿äˆk%^¿æ.oŸJ2©¿â󵤒 OTHERSNR3FGL J1805.6-2136eW 30?Ó+õðy™ö?Ðþ"f$-?æjÃ3?Ðþ"f$-?Èm—&Ë8a?Óî'tÜÿ1?éäš6M1ç?Óî'tÜÿ1?ݗ–ÿxܲ?ÀTܤÛ"?á44€C'§?ÀTܤÛ"?ºìS™p'X?´ëóú?ì¢uŒÑï´?´ëóù4FGL J1805.8-0803¿±*7?Ïm@UÔ¥ß":À9ůJÛÆeÀ;Šꘐ@&¦7aÁ@Åêû‹üù?È}ë=PBŽ?¨}¡%ãr?ätÌ?ß ?ý­:`N?ïû¶Å#‹ ¿éh°B¨q#¿ígB'¿ÒùsÍÅ¿á	²Û‰ÿ¿ïÿ‰kVOTHERunk1RXS J180603.1-080612?îø¯•¬?¢b¶õÅ¥? ~o5¥B?¢b¶õÅ¥?í[˜¾vÕ?Âdd€8?³#:IZ?Âdd€8?쮘qHüé?¦A¥‹Z?º‹<u¸¸?¦A¥‹Z?투A°6Ñ?Ÿø-]I$×?³ºò~I}?Ÿø-]I$×4FGL J1806.9-2455c?íŸ+µ»À¸Ðº%*À:o1çÙÀ;|`¾†¸ì@ÜHjÒÝ@"Á=L'©?ÔjßÇÑ:?êê!ƒ"@?úÁҝÇ@³+XžQº?ؔø T‡¿à39žeË¿É) 7mŠ¿éGF{"¿ïá=¼#1¿ïþ¼3!•|OTHERunk3FGL J1806.7-24511RXS J180700.7-245619(?Ñܘu4M?ÉÏóՍ?çø3ÅeÙ?ÉÏóՍ?Ö'ŒXÑpå?ÔûOÁo¡?äì9ӗG?ÔûOÁo¡?ÑzÖh²ÛJ?³u?/üX?çB"˦'[?³u?/üX?˱Tæ…Ñ­?¯iŠqKY¼?éªÆ^‹–?¯iŠqKY¼4FGL J1807.8-4340¿ê˜Eƒ¥Ù"À&G2œ4~À:4I½¹3"À<àd)u@§ÏBrì@ùœÝñ¸?Ãi¦!gXÕ?Ô'r 0Œ@
NHboa?ú:š³JÕ?ïù?†þŒb¿á8ýw"¿ÛxŒÙ—¶k¿ä½þ}ÉÚT¿î–q[Œî?"E©'oÜ\OTHERglc3FGL J1807.5-4343NGC 6541?Òã]`zr?ÊI²ÿõ8æ?æŽQOÂÆô?ÊI²ÿõ8æ?á#X׆¾¾?ӈjI¥»?ݹNPò'ƒ?ӈjI¥»?՗Le#?¹zz k«ª?å4YòsMo?¹zz k«ª?ޚØ7Y–?µ}'$áp¥?ಓ÷dS5?µ}'$áp¥4FGL J1808.8-1949c¿ÝPxÛ}H?]ÐСõ\À8ˆF"
qÀ9¶¡Ú°»@ –îE1b@àM/^?ö£©Ø«þ ?Ôôqâ'Ò@Ãñ[øN[?ø±÷¤;Þþ?ç:¶#£s?îêÖ£d!¿èÛLAw»¿êKåM¸¿çqµºa>¿àÂç 5)­OTHERglc3FGL J1808.5-19522MS-GC018?Îk•R1ˆ´?Ó7ûl4¬?èe«sÓ?Ó7ûl4¬?¡˜±yÁ¸?´ãÑOÁ¢¤?îætècï"?´ãÑOÁ¢¤?ʀ?÷Íý_?´ÏÛ8K?é_ð€¨?´ÏÛ8K?gi9Òó[?xAßUOi=?ïè–Æà-?xAßUOi=4FGL J1810.3-1925e?ªÿ¸wtj•¿¾(w~¢ÙpÀ7±C΋é®À9"y
2ª@‰Ä7@Š|Æ$<?À<"·Ÿ¿?ÒEkD¸Ã@¼«œÑ\@Öªß<;?ïë>bk]¿®w9>ÝW׿ÜèƒažÖo¿èPÄsa÷l¿ã#Îq»¿ïôU§ÒAOTHERspp3FGL J1810.1-1910HESS J1809-193"?"Kôóú§?°§DìÝ?ï] _p`+?°§DìÝ?¦c(Å]å?£Ô¥›c¸?ïzÌæ¹Õ?£Ô¥›c·?ÉüêS\?´ãÒ"§+?é»@úÅk)?´ãÒ"§+?"5Õ#G¯?ty'óTÇ?ï¯(«ráB?ty'óTÇ4FGL J1811.5-1844?渥\ÆA"¿¤lי¯iÀ8EŒîkóÀ9ã?¹SsE@+×IR"@ŽŽ¾tDu?Æ­'@
Üþ?Ý$)à¤&@ž¡aä÷f?ý	ø`Nt?ïû1~þá¿Ùv}_Ò"¢¿æ"ù2e-¿ê¶CŒ¿ïÿýF\I?ïÿ¨âaßnOTHERsppSNR G012.0-00.1?áê‡odL?Û6Ç­‹'?ÝÔ*ñ!7g?Û6Ç­‹&?º‹ "$V\?ÇjÎÃ߅'?쮋í›u5?ÇjÎÃ߅'?¼šùèx³?«™Íۛê?ìl Âðî
?«™Íۛé?b´r$Wî?WâÅp3Ö?ïíKñÛ¨?WâÅp3Ö4FGL J1813.1-1737e?ížñ•ÒÚ?Åæ­ýÀ6…Fü=ÔÀ9OVcÉÔ@f€®¼š@T¾ÆyÌu?©$S…í?Ã@y—Ɔ@µKHÓ®h?öf¼ýÌÉó?ïÿ@OÁß¿Ò2l"¿¿âµƒž¿åéҁ—š;¿çEsÝGnT¿ß:md1'ÚOTHERspp3FGL J1814.1-1734cHESS J1813-178?µèq¼-ö?ÂØ6«#?íBñÎHzA?ÂØ6«#?‰3š¯™³?©pL
/
?ï›1•AÁš?©pL
/
?Úr$ÝÙxW?·Pzß î-?âÆí'CÕ?·Pzß î,?:EŠ0<Pú?.bE¶¸&l?ïü·N¹øv?.bE¶¸&l4FGL J1813.7-1536¿ã"®~B¶"?ðŽw&¨
À9rp·"@À:¥Mçê_…@ ^)dÓ@Í`ÛâêF?Åꐗ'X]?.77¸º?Ï8ÿ%­B@Òͺ³p?ì/8"9³¿Ý#÷p"¿éÿJ-J»æ¿âåPQQ+¿çB:73rô¿Þb'|,OTHERunk1RXS J181335.6-153600?羅<äÙB?Ç·ÕDÝR6?Ђõ†6M{?Ç·ÕDÝR6?î7·A8?ÀÑ0¹µ,<?¦,"‹î,{?ÀÑ0¹µ,<?êÛnZ?³ÿí
3D?ǜ'Eʗ®?³ÿí
3C?î¹c¤?"4ؤZQ¶?¤iÎ¥¿ÞŽ?"4ؤZQ¶4FGL J1814.1-1710?äDñà4-?Ç	j!†ã_À8ò(zrÀ9þªhö‹@ ~JL)@¹åi|?Ð23Xòà]?·åΑs?ñftù§ k@½®€0'î?Û$cAmހ?ìÔ_¾+Ÿ@¿æE^XûÅ¿ê)óÿk°}¿Û]"3¿ëBÇû¬´)OTHERsppSNR G013.5+00.2?ÖoÈÇ)¹ü?уó±œÚ?äÈœk#?уó±œÚ?ä	+êìT?ր.VåLø?×í¨+Î'X?ր.VåLø?Ý·"õzžT?Åbë >?á$=…B°Ö?Åbë >?êeßËÓøb?µîÁ¹ý<‹?Æh€Ð°x?µîÁ¹ý<‹4FGL J1816.2-1654c?ÊfXv3#¿ÁS|©É½yÀ8FñTk'À9Ñ×rB<»@Ô_¾+Ÿ@Ä[^Ëgr?ÏJ*,¤N?ê[éhÐú@-?ü¿ÒxˆQô?îê?¤Z¾¿Õ4Îÿ,¿åÀ ·/¬–¿îo/˜sÿ¬¿à± ‹ü"%¿ïþLké]&OTHERunk2FGL J1817.6-1651cPMN J1816-1649,?½ÁZk>yü?Ά.ƒ•S*?ìGÔ²˜0Á?Ά.ƒ•S*?£‡I§"s?¹œ/Ÿ 
?îNjo•‡¸?¹œ/Ÿ 
?È3Á~φ?¸òeÞçJÛ?éó Lz?¸òeÞçJÚ?G¥wÍbt?FXœÎDˆ?ïú¿"§?FXœÎDˆ4FGL J1818.5-1656¿ž(Y¸cW¤¿ä¨ªxäî,À8×£Z»ÐÀ:^xèI*@ûÙc¯@÷‹7GN?ÆvÚèCuÌ?ٚcƒˆ
P@2 f<u?÷úÿåþÍ¿ïß4Bý«'?ïû>?*ã.¿à¸Gڊ%¿åz·\Ç+¿ìӋ,ïLT¿ïû¨LºÃ¶OTHERglcGLIMPSE C02?zš»0YÄ©?‹–Bå_Ap?ïÊʉŸLw?‹–Bå_Ao?œ5æd?«J³¹y-Ä?ïNPÌÛ?«J³¹y-Ä?­áÉ©:7r?ž*ò
?î!ãel\‰?ž*ò?‰e3àXÝ?x(Tðxì6?ïšiû0~œ?x(Tðxì44FGL J1818.6-1533¿îb;EÒ¿RnóÞ)YÀ7^²²$«À9^[ÿÛ@"ú%u…h@;¾òïv?µ7ƒNÿl‡?ÒÿßÝ5¦@1í¿‹›ª@‰a´¥ä?ïÿõ4Ê㿽ë *F>¿çìÞ²þE¿éçÑ—Êâ¿ëŽ5Lèæß¿ïÿò~#¿OTHERspp3FGL J1818.7-1528SNR G015.4+00.1?½ˆY=÷?ÑÔùP¢ðÕ?ìNôØP?ÑÔùP¢ðÕ?|%(Zér?'Á ÔÀ?ïǵ¯J-?'Á ÔÀ?¿Fnåáf?«±š`BŸy?ì2#CÓ<?«±š`BŸy?;¾ø"9 Í?.Dµ•QÅ?ïüˆ ïxÌ?.Dµ•QÅ4FGL J1820.3-1009?²ù&oÖµ°@zÿèƒÀ8òdtJÀ:®nƇ8n@x±Ü¤Û@^YåN£Ò?Ç=|!äI?ÒTÕd éo@KBôqW?ó	Gðjâ?ïÖ8ñ¹`¿É68¡1=¿äÛ
bY'l¿åépq'#[¿ê#u –
¿ïÿð懈öOTHERunkFK Ser?¸e–m Ó¼?¸—Õ€Wz?ìóM2Kå‰?¸—Õ€Wz?¶d@
?ÂIÚp{?í=wþ^?ÂIÚp{?͖'g¶ž8?±]ßÛmLd?èš[¦Xs?±]ßÛmLc?‰ã-w¶&L?tÈýá'ÍO?ï˜sJ!'f?tÈýá'ÍP4FGL J1820.4-1609c¿é´H㒂ª¿å^®óÀ7vÀ#jÀ9ªdÜ"«&@lúnp ý@RnÚ©.b?°Wá&öå?gêfß´»F?³£</±š@Ý<¥wÉ:¿Ý	üƒ×+¿çµv¿åªÒa6PÊ¿è{:3µ¿ë¿Ôj³w"òOTHERbinKleinmann star$?Ü÷]ã© /?зé;æZ]?á"Q+oè?зé;æZ]?î<
†Zð?·€¶?¬?WžšQ	?·€¶?㥁ݶB?¶òÇöVß%?Ø´ýèD"}?¶òÇöVß&?ìMÖÓ7"'?°'c6íÓ?½'IfFëu?°'c6íÓ4FGL J1821.1-1422¿à×3}Kv\?™ÎWçG¢VÀ7"H¤´ÏÀ9Y{ÕctD@§i&à@M¢ÝåùÄ?¹Â|ò–‹?Æ®nþ:ƒ	@
ë€ìúi¾?óÒÑ=õ®î?»›Ð>ò.¿ä(@zi¿æ'ñ.«äö¿êAyHªi¿ëát#¾K¿á»]¤ YOTHERspp1FGL J1821.1-1425cSNR G016.7+00.1?ªR
×؜?¿€âÏð"E?îZß^2'w?¿€âÏð"E?¹Ð8¾X—?Åwý_$Q?ìÅÿxè4î?Åwý_$Q?ˬ֒ü‡q?´Åî"mËï?éÊ[@Þ$?´Åî"mËï?zó"|œ©?hóV!I?ïÊ»ÛÇ?hóV!I4FGL J1821.4-1516¿îï
ø—X»¿Ý5%:ÍÀ8Iûçl‹DÀ9¢*9mÇ@Épgq(a@ŸGù"Õ4?ʹ~%õ²õ?áõ£àðEM@Bþ'Q@ïƒm2?ï½'"ƒ¸‡?˜hÀçCú¿è¢Ë§2ßP¿ëW*ß&Á‹¿î˜ìËoÕ¿ïÿA"VOTHERsppSNR G016.0-00.5?¹ô†¹T?ŗ¥•#R?ìÁo?èݖ?ŗ¥•#R?¸²Šüúæ?Æw‹ô"®?ì鮿`¤?Æw‹ô"®?Æ­_ÀÕ?±O¦Oˆ?êT¨»OË?±O¦Oˆ?†ŠÛ§òm?u'É\Z†=?ï¥Ô'aø5?u'É\Z†=4FGL J1823.6-2345¿çÜ[žœÄÀ'ÛŸ'xÀ:&Mâ"sÀ;›mB"º?@Ã=¾Q‰à@;Û¾Ø?Îø¾'²!{?Ѓբ‰WW?ü'à@bMÖøtÆ?îøçþ¡f¿ç¼]éÀ#¿áä=Çᬿãù2±-4¿á_Cr¿ïø°ëŶXOTHERsppSNR G008.7-05.0?ïJ.\¶U½?¬äúPNþ?–º4i5HH?¬äúPNÿ?ïö¸Âaž?pd¯$¦ë?RŽ{=ÌÅ­?pd¯$¦ê?뫁pÀmw?ª"º€2à?ÁQú<þJ%?ª"º€2à?ï]á÷(Éê?ôÞ3
?"CÁæÂÃ?ôÞ3
4FGL J1824.1-1304?鶚wðÕ~¿q™JÞ-näÀ8ÝäLESÀ9'ý÷Cõ@ÁªKÃwä@|5À¬-?Ëó²ª6ÊÂ?èh(=5ët@"£Ÿ¬Ù@i'|'v?ïøʁ˜ñÔ¿Þ1›cHNοç(¬âKº¿ïÿ¨âaßn?èÉâÂW}ë?åÙÑ,­ÝôOTHERsppSNR G018.1-00.1?ëhDú‡Õ?ÏVãá>ÇÚ?Â]úìàª?ÏVãá>ÇÚ?ÐÔÐa¸q?ՁY'Š»¡?畗Ï#Ç|?ՁY'Š»¡?Ù*¹(û‡?·Hd*"Îv?ãj£7ë'<?·Hd*"Îv?¶7§Ë'Ç9?ÂÚAvôý?í9§?ÂÚAvôý4FGL J1824.5-1351e?Ò0§•"'(¿Ý6syÀ6³"÷si"À9N?(3ü@#›Ÿ"X·Ò?û¬	sFHº?¤å¿b%??‹R·ƒ#?öŠÙv0@äÖ¼9ג?֋Ⱦâ(?â6*~®±¯¿Ú³8ÜÀ_׿ØcµÜñ22¿Ùsßà›¿ÌÚeçr~OTHERPWN3FGL J1824.5-1351eHESS J1825-137?戱	‡d?ÌÎ#ÆëÈ?Òîìñ7Ç?ÌÎ#ÆëÈ?âØ]ë®G½?Ú_))Oaé?ÚOD(£p"?Ú_))Oaê?æ˜äѦ-?¹¢uB=î6?ÓØÎ6\³§?¹¢uB=î6?Û3×>žø?Ém58C&p?âft`°"?Ém58C&p4FGL J1826.2-1450¿ØË«š$k¿ô¦D¢Ç?ÅÀ6 a3÷À9i£bp7¡@ãR™€@J© öÍ?–\Û£)eT?¿gûfé2@ ¬B 6m@›6PtÀ¿ÖdΡ8Is¿ä ¹ÿȏ¿æ{4ßZÃñ¿è›Ù°
g¿ìwQ­Dq¿ØÇ¿Sg†OTHERHMB3FGL J1826.2-1450LS 5039?¡; Dû
?¶.³n‹WÆ?îìMû°O.?¶.³n‹WÆ?x°cºÁo¾?‰)>m–?ïΟ8Š}!?‰)>m–?ÛiýÊLÎ+?´ñD‡b.‡?âK٘ê?´ñD‡b.‡?7Ó¯+xñ¨?)aÀlþ2?ïýŠá?)aÀlþ24FGL J1828.0-1133?ÚOqèU¿ÂfS†ÑšÀ8Nµ‡5éÇÀ9îÐ_(""@&Þ÷q@ö¥†6æF?Ä/fÉû?âtöL"'@'5Ÿôým@eãmx(†?â ÀaŠ	?ԋ"|I&º¿Üi'ûr}¿êfs.ËÅ¿îrç;
¿ŸzSƒ4ÓFOTHERspp3FGL J1828.4-1121SNR G020.0-00.2?r™q™3‹?°.Y,"š&?ïÚÍ͘é?°.Y,"š&?'É)ß|v?¡×¸©""?ïi¶±P?¡×¸©""?‹Š8ð¡¹p?y}Q}~‰?ï'×=y?y}Q}~Œ?p×	'i ž?Z¥Ë¦è£Á?ïÞQìÛ-¾?Z¥Ë¦è£Á4FGL J1829.4-1256?ïë¨Ó>ß¿ñeªIFÀ9cQ³PúÄÀ;ƒ:=°@¼]¸ÂÔ¦@"¯ûî|?ÍÛ`#`"?ïÛ}i¸*~@õo›Ìz@³ɝÃJ?ïƒ{_œÈ£?ïÚËB‰Œ?ˆ¢õ¸ÔG¿è¹"8à¿ïþ>>ª	Ô?ï¨wÆOOTHERspp3FGL J1829.7-1304SNR G018.9-01.1?¡B·Oj¶?°š¾×gz5?îëÞô‹	U?°š¾×gz5?¤q3«³F?¹1î³]ýG?î¸ìÅDÏ?¹1î³]ýG?²&æ4'? Jîòµ?í»?#<ùn? Jîòµ?VE˜çH'µ?O³Ñ(ÖÉÝ?ïôÝ3Œ[·?O³Ñ(ÖÉÝ4FGL J1829.5+4845¿Ñ³.›˜¿@7Š\å´$À8¾©@'À;ûl'à±@B˜*Þ@ÙuòËd?¡òœ*'?¯'öiÿ"5@êeÀN9@ë財*¿ÄI'C¼˜¿âßwßµ‡·¿ç›˜w[¿ã".ülοë€JœÜD¿ÞU3ÃÑÑnOTHERcss3FGL J1829.6+48443C 380?ïó6Læ'?Wñ´V±üZ?Y"ûf2Ü3?Wñ´V±üY?ïõܯç?r»PžÙû¾?UÜF 1ÞD?r»PžÙû¾?ïq]8[
ö?Žs"ŒÊû?'ÔXôž¡L?Žs"ŒÊ÷?ïÝÓÖ¶ô?_¸1úeŸ¨?qô$†7?_¸1úeŸª4FGL J1830.2-1005¿ìصäø?«W2"Ç{À7×)ž^û8À9""išÎ@¢ÌÉè>@
Å㤀?ÄA¼bò= ?Ûæ€<¦N‰@ÓÖ¿•?ôÈ[á¨&$?ï±½¢bk¿ßZ¿žæàt¿è˜8p‰Õ׿옝?ìT'¿ç?Ô@ßn:¿ïÿ·ÀÌ
ŠOTHERspp1FGL J1829.6-1006cSNR G021.5-00.1?ÂÞòX\Tü?Ð_ç°:'?ëHCièêÁ?Ð_ç°:'?¥‡ë€$[á?¹øâ«@
¡?GýºB?¹øâ«@
¡?ӆ&ÕÐ,'?·)ËN™À?æ<ì•é¸?·)ËN™À?@àFî	F?5H^?ïûÇÜ.D}?5H^4FGL J1831.8-1503?¥Ô"H­ÚpÀÈõÝgNÄÀ:™ °åºÀ<RG—nF/@ÐõLrÊM@Ê}Å'¼Ý?Õ8¥ƒ1Î.?ïý'ÒÕûJ@ÃC·õf?ü€Ó6ô2í¿µL+@V?ê?ýkûý?ä`s^™¿åª%mwҟ¿ï$X*Ž¿½pc×%ÁOTHERsppSNR G017.4-02.3	?¿Àwµµ•	?¾k¢«[2?ìñ	IM^?¾k¢«[2?Ò)Pš¬n?ÓÕ2´Á#²?æëWú2©É?ÓÕ2´Á#²?Û}/kr85?»Ä¦¾3†š?âAhJFãæ?»Ä¦¾3†›? ÜŸ¼Ùw?ˆäµ€?îò6?rh?ˆäµ€4FGL J1832.3-1433?à™Ñ'ñWÀ¼,†pÇéÀ9ÌEŠMÌ<À;=5¾(@]l²ŒÛ?ÿSýÈîû?ЉCá`x?ÙmR=åhÐ@ø£ë,3@À<-'Å¿ïxvétù?ì®ç¸5f?ÒP×Þά÷¿çŽáDS(¿á4&¾Ýà¿ï÷åê«%OTHERsppSNR G017.8-02.6?ê/µ)h'?ÃùHfo?ÇA+Z_ûf?ÃùHfo?îÍêC-î&?¼ÞS³­#?£![Í!Ÿ?¼ÞS³­"?ä
d^AP?¶IZáÑÃ{?×å7ûC}`?¶IZáÑÃ{?êÚ*Þ#¸?­Û¾Ç%?ėT‡q˜?­Û¾Ç$4FGL J1832.9-0913¿éì'Ø"¿ÁÁ›o¨ÚÀ8Ó^R›®GÀ:†••þÚf@h'Ô±Ã@û]‰H¾?Ìwt«£‡Y?å·Y}ʱ@Q['—@¶HW²™p¿ã€üŸxUÒ¿×xû~æåÓ¿Ôîÿ&¼,l¿çXUÌ»/¿î–÷'ê)Õ¿ïë;³´MOTHERsppSNR G022.7-00.2?u¯'|àl?"»;XpPj?ïÔ¡Îû??"»;XpPj?¡€Xo&T°?µ6ÆC)¿?îçúy
šµ?µ6ÆC)¿?±0÷€r·6? ÷M$3Óå?íÙáñ©? ÷M$3Óå?›Fí~À÷
?ˆt"a!Â?ï%Ȕ	øH?ˆt"a!Â4FGL J1834.1-0706e?ìáýVæ?âºíÜçÍÀ7‡†Nc:bÀ9÷‡©­
@ ºÓ»ÔW@B¤¸±?ª6CM1·?´¯Ï;#@½M%LÀ£?þ8r_˜ìË¿ï}1NV¥(?ïO¼5¥Ô:¿Ø_~Øտܳ@S'D¿ä…|áÒîO¿ä˜…2ˆKOTHERSNR3FGL J1833.9-0711SNR G024.7+00.6?ÙMéÏvÇ?Ð>™TûT?ãvÙDœ?Ð>™TûT?©øø;Ý;n?Ã>[(–#V?î`p|B,I?Ã>[(–#W?âP9ÿŸ6?½åßîW?Û_ŒÁã"?½åßîW?µD…ƒn¼?·òfQ7‡?ëR®ÞŸ$P?·òfQ7‡4FGL J1834.5-0846e¿ÖÞ"*¶¿ÑêÛá<ÆZÀ6øêúÀ9´ëvÛÿp@!q3­ª@øã["‹?©ãZ> 2a?¡7ßÀD~4?ö˜ÏTf‰¢?ðX#…@FA?ê!j³Ó¿×AIÌR¿Þ|cÓº¿ßü
1¿åèå1G ©¿Ö¿²ÝãJ"OTHERspp3FGL J1834.5-0841W 41?څ,E?ÒÇ]¥?â½qéÿÝ}?ÒÇ]¥?Ɨrè‡æu?Ó Œ-§E?êZ#EÞb?Ó Œ-§E?ä#Ø7¼{?»w÷½¨Eâ?׸O‡Ç?»w÷½¨Eâ?™æ¹/9?".€Ò€<?ï7ÿøÊ6†?".€Ò€<4FGL J1835.7-3258?"QìØoÙÀ&¼q'êRðÀ:"¾@BÀ<#=,±8ó@³7ƒ$O@Ê#9Àëî?À‹ön?×ÍýNtØ@R° ě¦@J~}"N?ïÿ?`h¤¿Ã—Ëù")h¿ãmß âM½¿äQQ¿î;Äf̽³¿ïûç6Û^`OTHERglc3FGL J1835.7-3258NGC 6652?š˜tä¦p?ž@š¾†»?ï+<XÚό?ž@š¾†¼?­ðGì°?±`&û
¼¢?î ÿ†!5?±`&û
¼¢?© '¦g?î?Kt?îmöåŸþ9?î?Ku?Âi¹ÉeÖ? ¿³æw`?ëe¸Ñ¦‹? ¿³æw`4FGL J1836.1+1143¿äSkî"†@!\^Ô¡­dÀ:uOøÃÌÀ;ôWVP@Iބ…5_@Úµ€í ?Í°£vg:?Ð#Ëâ5!@­Ácâþ?út"« «¿ë¥C¡?€I?ïôἩi¿ÝCm¨z-¿çrº'Gm}¿Ý‰šÈïÿð ¼x—OTHERunk87GB 183342.2+114143?éÊ6F'?Ã=ïÄ·p½?È×&çϯf?Ã=ïÄ·p½?æɽcaZî?ÐSĖëky?Òl…9=J%?ÐSĖëkx?åëËú›p"?·ÓR'éâ,?Ô(h
É×?·ÓR'éâ,?ä±3œLl?¸"¤I8?֝˜zÇg)?¸"¤I84FGL J1836.5-0651e?ïÿúru'?ÄCO¢ÝÀ6A‹sf)*À9"Â(.s@!&¤†‡™@;ÌDÑ	?›2Gk'í?Œ8e!Aï?ñ8^€¾×A@9nY$¿áµþŸWɖ¿–¦…Üàc¿àÔ*ÄϨI¿áÖG4q÷"¿âÃai&Š¿ØuØstOTHERpwn3FGL J1836.5-0655eHESS J1837-069?â^ßµ–?ÑÙ¢YÃÖ?ÛBAûú"Õ?ÑÙ¢YÃÖ?à{Û9«~f?ÚPÛ½ßø?ßIŒ©2?ÚPÛ½ßø?äxR$Ô4?¼"YëP]?×[¶W–þ?¼"YëP_?× ý{E֙?Ç|"Ì&?ä/B]³?Ç|"Ì&4FGL J1836.8-0727?ìF6¿'¿Æ¡)ÛƏÇÀ83È-*ÛvÀ9õ}å-@¥ˆáe‹@8ƒŸ\Q:?ĆÒíx=ÿ?ÞYG™ò"í@I[»èxû?õŒ>Ù.°¿Þ†=0âöÛ?ájÅÁ?Ðпáµ'ÿùJ¿ê½®ˆ*Ü¿ëleöÕ¿ïÿð°×£ÀOTHERunk0FGL J1836.1-0727NVSS J183652-072453?²¦Á$Ûf?Ïr•ùÝ-ª?í«'Ûd"??Ïr•ùÝ-ª?'×iZ¨¯Ó?—ñæHˆÆ?ï´¢Z•]B?—ñæHˆÇ?Œ—ŽàLhÎ?}–ҝ ù?Ä~Î\?}–ҝ ñ?,ÞMBnZ?*/v9?ïþ2'ëÙ?*/v84FGL J1837.6-2904?âKý¼%çÀ$"¹,HÀ: š=-‡ùÀ;ÞËêN½Ó@¢Câ-@Qš&‡S?ÌÇ`|B?ÝÙoØ2@4f'ëØ+@	…nVŸÉß?âó\²¿Þ¼l—ØÏ:¿äJ½"s嫿薣L;¿ã%žÀJ‹¿ïÿ-<y-OTHERNOVV5668 Sgr?ë,
pd€?¿ü‡ÍA)H?ÃOÖ>o'ÿ?¿ü‡ÍA)G?âa>hj³¸?Óì?®4ì?Û=ƒ/*˜?Óì?®4ì?â×H"}3?¸àkyܦ?ÚQn÷™ï?¸àkyܦ?ãÈÅèìc?·=ôÔ¿^±?Ønt.'8â?·=ôÔ¿^°4FGL J1838.3-2148?êÂú¥X…ãÀ‹;26À:h Ä0FÀ;딾h…û@Tñ¡˜kœ?ûžƒ
f?×µ˜ñ/?îªâ+Ù¢ž@&ó|cþ­?óZ…tɀ'¿éK—¾":?ïÝIúÑÿå#flE£x¿Ù££Þ–ú¿åñ0ߛÜj¿ïâÁáaYaOTHERunk1RXS J183818.2-214857?ìµù•ÛÃ?¸§ÌSñyÌ?ºP3Q$ç?¸§ÌSñyË?ã±°<#?Öïò:U…?ÙȜŸ‡¹Ô?Öïò:U…?èGêÝ?²eÄZÏÎ?ϋ•ŠàTˆ?²eÄZÏÎ?ÀF9˜Jû>?¬y1Ž¤ë?ëîq™íA0?¬y1Ž¤ë4FGL J1838.9-0704e?ïÜDU˜Á¿Ý¿í@_Á‡À7c½ZiÀ:
²p*4‡@"EÑ4O?ýTç4?ª­ƒö?ž%.§w§?õ-ÑD*Ò<@SÖK¦¿äWLíï\D?ìÛÊ`áÂ'¿Òé,êCÖ¿ß4<Kµ¶¿ÜÔ–j:¿Î¿r[½OTHERpwn3FGL J1838.9-0646HESS J1837-069?ìñ¸Ÿoyo?»ç]Q©[?¸r;"4"?»ç]Q©[?ëkV"ׅ?Ð0ÀÎð?ÂR§§t¡é?Ð0ÀÎð?ç<6u›}?·0"TÂ$?чû"É?·0"TÂ$?ê†c"TGÑ?ºfû^ôø{?Åæsv®àº?ºfû^ôø{4FGL J1839.4-0553?צ$N`ù}¿›8g®´À7Eõ­–§À9T'œýÒ(@c;'PŸÖ@Ð:?–îÄ?¯RSÈ)$?ՖBÚ¶@(dÀ
¡©@Ë#œè-¦¿ØœOAÙ´?¢b`¿ªÇ·¿áÈÖ"‹ñ¿å¼žK°»¿ì'ê@%4¿ïÿôým~‰OTHERunk3FGL J1839.3-0552NVSS J183922-055321?Ç.¤ªBqC?×nÜÄ>?ê4VÕoc¯?×nÜÄ>?V‹ÇŸ¿¶ð?féýêG÷ë?ïôº0 %?féýêG÷ë?˜o¬¢h–?"ØöoNf?ï<'šì»O?"ØöoNd>óЁøwÓ>ñýËAW_?ïÿØ^ü>ñýËAW_4FGL J1840.0-0341¿ïêIò|é?ëXéÀ9iS$jB"À;?Ú˓é@ŸAЄè2@Š…) ?ÌÖßuEý:?êù¬ÿ§ël@Œý©äj@'bˆ‹T\¿Öüz$r뿧Š
¿Ó‹‰ þé¿å»;u!M¿ïúøÞ£¿ïÍQ!ZÛOTHERspp2FGL J1839.7-0334cSNR G028.8+01.5?i$/hs}!?lÔ/CD?ïæÛЗŒƒ?lÔ/CD?…ÉHǖ5?¬S§€Õu?ï{ѵ¹ÃN?¬S§€Õu?¤󡸳ê?'ɇ$Æ3ˆ?î¾ ÅätÁ?'ɇ$Æ3"?}Ø}ª¼u?hH'*‹´+?ïÄOª‡?hH'*‹´+4FGL J1840.0-0411¿íÍ
ÄâÓ?ã²â`1îåÀ8Ë6Z/ À:¯X¶zzð@§qºGº@Â…îÁê?ÀéÁЈg?ÕTpšœÏ@T´:ç?û£gΛY¿ëDä þè©?îAÔKFOp¿Öç¨ñ%r¿äd˜0
¿ìÿ"=ßßy¿æ°Ë¡ÖªOTHERspp3FGL J1840.1-0412SNR G027.8+00.6?iù8}˜T?hY")"Ê?ïæǂgp?hY")"Ê?ƒ"sP´o?Ô€ªåO•?ï±®2½.?Ô€ªåO•?¥Ã{¥³P?˜…q].?î£ÈO5¤Ë?˜…q].?ŒõF0Góz?~f§?ƒŒ?ïŒ*ç>à1?~f§?ƒŒ~4FGL J1840.8-0453e¿ã܈.a¿y?¿¹Ÿ'À7Y…tH§9À9'$~d@ˆ¾)pçŸ@úh±šA_?³uÏ:p`?Ð4°@¥¾@	G{À?ütXåIpa?îfKŽs˪¿ËOøæ±${¿áç—Sn¿çá}ÿ	_û¿é¹Ù«¡¿áĖgµñ¿OTHERspp2FGL J1841.2-0459cKes 73?r'ä+w/V?§^ƒ	b3?ïÚú7©¡?§^ƒ	b3?€(ì'ºÍ?…½õYŸ×?ï¿\O…µ?…½õYŸ×?²yS~ÊÌÍ?¤n
/¼§?í°Õ&¦f?¤n
/¼¨?OûÉ3æ?=צm—¬'?ïø
³\?=צm—¬'4FGL J1840.9-0532e¿·@®¿7¿Éc\ɯŒÀ6ÁHO$*'À9¢ö{@!À¤¿:¾?ÿžá¢FçE?¢qNCQZÞ?~¢¨¿"?Þóå÷1?þ8=ägF?çÞ&'dA¿¹j"Þ|L­¿ÛO
*á¿ààÙÿ»6¢¿ãäkß÷÷É¿ÓKA\k»»OTHERPWN3FGL J1840.9-0532eHESS J1841-055?ßð3šL"¸?Ñ1'*¶?àæ2Ù½¤?Ñ1'*¶?ä$ÜìÛВ?Ù
ŒÏ+qú?׶F&H^Ú?Ù
ŒÏ+qú?äԟªŽª?º½–^?ÖVÀ«Òâ¬?º½–^?ÔÏÔÔòŽ?Ä×Z¥³?嘕ô†¹?Ä×Z¥³4FGL J1842.2-0751?ï(R¿R¼¿ø֍
?#À9m‹U38<À:í‹ÿ}#@an"B€@]™`Ž¶?ÐL]їb?Öļµ'•?ý*áU
È?û¢£h¥Zî¿ïúHÿÏ?ïÏف¼O¿»³¦
@JÉ¿åÛêaˆ0;¿ìXG¢'v¿ÇF£¨f;OTHERsppSNR G025.1-02.3	?ÒÚhB¥æ%?Ƚ,ƒ‹_ ?æ'ËÞ­î?Ƚ,ƒ‹_ ?â•Twp8?Õñ<·Š—{?ÚÕWɏ?Õñ<·Š—{?ÚΘZ&Ö'?·2œ®Wuõ?☳Òì"í?·2œ®Wuõ?ÓúnñaÞ-?¼"z•[Àñ?æȇOé?¼"z•[Àñ4FGL J1842.5-0359c¿ïÚ¢Ä*-õ?Ãå>]³ºWÀ8
°Úþ¾·À9Ÿ»	Uê@Ýp3Ü@jZaueÞ?ÄèÀHZå?؅ZZna@\äŒ×ê@‰Ö€TÏ?åi¹×ý'w¿á<Ó$Õ¢^¿å€™¸£J¿ê?*b{ö¿ïþmž"ÿQ?ït4à‡iÁOTHERunk3FGL J1843.0-0359cNVSS J184240-035858<?âO*8O« ?ÚTŠ©ýü#?Ûa«`¨Á?ÚTŠ©ýü#?Âx‹»êuV?ÌèópüÐ!?ëaÝbª?ÌèópüÐ!?´hRíŸT?¤~;g8Î?írõ¼BL?¤~;g8Í?•6"‰°ßT?Š¹°ÄF|ð?ïVKÛ²y?Š¹°ÄF|ñ4FGL J1844.4-0306¿Ý‹ù÷ð—?À0¸@¸À7±Ÿ°4ÒÀ9zh»«<Y@KŸÅÒ=@K9âyÝ<?¼@|ÇÑ»I?ԗ?a¿¸'@7?tN†@k%ПX?ï%)œ±|¿â0öýø¾Ã¿å'0^—ÿ¿ê–—†™ã¿íïßáÒmv¿ïöÁ'ÜæöOTHERunk1FGL J1844.3-0309cNVSS J184431-030716?s¤Wá¸?¦jÇñKÔ?ïضýQÐ=?¦jÇñKÔ?ƒ®á¹?Ž¹ì%7C¯?ï»ÑóýDy?Ž¹ì%7C¯?˜¼èêɁ?'v-¨MZš?ï:¸©·T?'v-¨MZœ?;aÂ
ªêq?-п×ØÛ'?ïü"ǾJ£?-п×ØÛ'4FGL J1845.8-0831?í"c)tY\ÀH㞠jÀ9ƒºéuzÀ;RALÑiê@#ï{M~@©"˜€•?Á"©…JV?Öå-a4l@PÔ~qõç@û†°ð?ïöׂˆ[¿â±Âëc'¿Ýt^ÁVw¿åÞ¯îo´Ä¿êîU'ÙŒ¿ïú–ŸVOTHERspp1FGL J1846.0-0831SNR G025.1-02.3?²Ðsâ_R?²/Á‡¯?í¥ñžã´?²/Á‡¯?Ö-+BÖ²Õ?Óÿœéú®1?äéj^"¦–?Óÿœéú®2?Á(†r;¶¯?°Þ5÷"?ëµÞcqT?°Þ5÷"?Ò¢Døî.?°¿ƒ"QE?æ®Ýñƒˆé?°¿ƒ"QE4FGL J1846.9-0227?ØLÎx8k¿½
ò[ýËÀ8ï͂Õ2À9¥rE—¹Æ@BAê04ü@R+Ù¢ž%?ÁƑIhÿž?Ó'mb*W@Á"tŸ@ŠÒÒË?¬ÄÉ¿Òu`Õ,î¿Ú-³Âd¾ñ¿èëð«Ï¿ëîÈáÉ¿ëW€OE¸qOTHERunk1FGL J1846.8-0233cTXS 1844-025?s*¢€.¢?§>5%ü4d?ïÙ«Ôºÿ£?§>5%ü4d?-°Æñ?¤·kr5=‰?ï~'yÈs‡?¤·kr5=‰?‰-²"UÅF?wÁ¨ä\?ï›I7v¨ì?wÁ¨ä`?mÁŽI€g?`B["Ç?ïâ>q¶ç€?`B["Ç4FGL J1848.6-0202c?éø(§ëÌí¿ÔQlĤ_EÀ8RW˜mI¯À9¤mvûßà@ôüî@ç¶ãV|?Êk¿m"¬?ל;À•G@TUêî @z˜v. ¿íœ"N‰{?ï-ÇW嚿Ú<ßï¿@¿êh{œ"÷¿é5BEî¿ïÿ*±0OTHERunkNVSS J184840-020408<?¦5^jjÃ?À¥oê;ã¯?Y^D?À¥oê;ã¯?"*­jÁã›?¤ýõ×>ט?ïfª"©ðã?¤ýõ×>ט?¶Tñåà{?£R
ÛL?í5aÃ_Cð?£R
ÛM?…]g¢?|q¯@¦?懲‹ó¾b?|q¯@¥4FGL J1848.7-0129?ïÅP«±;t¿¸}P·
HÀ8'ØÚø	À:S‰X@úFô±e@ND¬{?½©O€W–?á1Ú£O%@"]Ç5ï¦?ûøýlÒ¼%¿Þ›C<뙿ÛwŒ>] ¿ÓQGpĎ¿âgšþôgF¿ïü¸Lã¢?æ®&ïXOTHERglc0FGL J1848.6-0138GLIMPSE C01?Ë]]à¹??׫Ë+Õ@?é(¨‡Ñº°?׫Ë+ÕA?tnõ¡ó?•!ï·Yñr?ï×"æ¼?•!ï·Yñs?™Ž#¾ÚÓ?'"€"»€?ï3Žâ)?'"€"»? ¹ßÄé"?7ÐóI"?ïþôb±g?7ÐóI"4FGL J1849.4-0056?ìڊL2¯
?'|[p>+ŠÀ7€3)'°À9¥€(¯K³@£‰™o@-"œ)–Ò?® è?Â&ÕøÎ]@—»s5@|s³Öܛ?ђ'ýîØ»?ì›Âhż¿àKH¾4Ù|¿ä'É oâ¿ç~þþx@ƒ¿êKý>¯"+OTHERsnr3FGL J1849.4-00573C 391?ž*à…*ÔÕ?µ:3~eã?ï¨ûÖ©Z?µ:3~eä?…ô"Nlû ?¤5³š??ï¨-îÆL?¤5³š@?Úݽ³FHq?¹¾ö2F«?â'!&\ÛÈ?¹¾ö2F«?ƒøŠº…J¬?yÒÁúsØ?ï°ÕêÕ?yÒÁúsØ4FGL J1850.3-0031?ã;Yº¿rä{_ßÉÀ8Ú¬è*÷À:A
±3ê@¤WZn@g8¥Ì®?ÈÔÌ`it?ßÅi`ì©â@'ã'÷Ó@'Ź2;<¿çHGä¿áx{Â=ä¿Ûí$S†¿é_þ"/T׿ü¾, ¿ïõEâb`GOTHERspp3FGL J1850.5-0024SNR G032.4+00.1?'mV÷ã¼? >²ª‹o?ï¶J¤#¬r? >²ª‹o?¬ÓQdƒ(??¾Àñ`0?î2Êé·Í|?¾Àñ`1?¤k"«–t?–IW
ü\d?î¹FµO¶™?–IW
ü\d?Ÿ««üÊq¶?ŒÆ•2'¼Ó?¬r?ŒÆ•2'¼Ó4FGL J1851.8-0007c?¼ÿÝS[¯Ô¿Ã·—†nïwÀ8yN»NöÀ9ß:~_@UE®
@¥¦½n‹?Ð?'}rq?ƛi÷?'@hýAߞa?ø´ý먰
?ìûi,êCÖ¿çÈâ\¿ãÑ.~§¿ë5*Ø>¿éSÕj*@¿ïÍ;]ÎOTHERsppSNR G032.8-00.1<?ȇ3¸_Vz?ÉäcÂ[^ñ?éÞ3è*b?ÉäcÂ[^ñ?Õê&]S®?ÔG¬_šœ?å
ìÑVtª?ÔG¬_šœ?ÓïÙ~Uã?¹œ1§Xg?æt@Õ?¹œ1§Xf?°o¨¨Îª?œ]Ѩ(߆?íò
êíæ+?œ]Ѩ(߆4FGL J1852.4+0037e¿âz+ÙºÒ?²¾vrÍýÏÀ7*'U¯^þÀ9n@V1dý@Ë£Œ·ˆî@XçW'Ž
?³uÃ?t#?Ƕ›Ø'@¹DŽO¹@&;Á!Gù?ïƒ9L¿ÚFÿøš¿á>f7l}Ø¿éâŽÕñ9¿ç֔–ûY¨¿ì‡{‰äðOTHERspp2FGL J1852.7+0047cKes 79?³ÝW:FöŒ?¾ß1li?í"U·!.?¾ß1li? S­)Û?³¦¬ŸŽ?îúÅ-bN°?³¦¬ŸŽ?ÖϸéTN?¶ãý#g¢@?䘣‹UÙ?¶ãý#g¢A? œ"bšÉD?ŠsÁ1@}?îö6¹ÖSl?ŠsÁ1@}4FGL J1855.1-2243?î¦i¤UfiÀ%цÛPôÀ:f	{¸À<C{cM­2@p¾†¸ìE@Èêí+?ÅGmgaŽ?ÙÆüÿ¦@ ü ÏîÀ?èÍ®z§?ïÑGP ©Ä¿Ü´'drñ9¿ÜÊ1ç٘¿àÿà?Æ>"¿ìAÿ~Ñ¿ïÝv¾"eOTHERglc3FGL J1855.1-2243NGC 6717?·ûÞsœ+?Ÿ[èYf/?íÄ1Œ{?Ÿ[èYf.?Ä´0-?ЋÂU>vÜ?êÄRRóô?ЋÂU>vÜ?®(x*m? +ø+Ñù"?îmx}Y/? +ø+Ñù"?>Mgl'Ö?{ÇßÂ}p?ï~
"Ä›é?{ÇßÂ}p4FGL J1855.9+0121e¿ïÚg·gøA¿ØÕ[½•øÀ5pfB
gÀ8¡%µ¿j@	-%R@ê쑎2?™=#¡ð«#?ÎÝöjÕâ@8oÏå†6@
Çf,"ÃI?ïÀ°^×ü¬¿¨šÜ æ{0¿ã^ FÇe¿å׈b9°ü¿ëS€™¿êP="OTHERSNR3FGL J1855.9+0121eW 44?"ø†(ĀC?¦Ä‰Æ¨²?ï`;ιÛþ?¦Ä‰Æ¨²?Fg-éHÖç?Weö –æÊ?ïúf4…­Ë?Weö –æÊ?º}6E;Ù?³MWB¼}›?ì¿°Y7X…?³MWB¼}›=ù‰rIº>
\|ãU3z?ïÿÿÿÌíç>
\|ãU3{4FGL J1856.2+0749¿íª¯‡ôÓÚ@ö>e–\ÎÀ8v(]íÀ:3ùÄ|œ3@&#«UÚ@(îñºÂß?Ù¥"Ò?Ò^zښ@{ؾr–ö@á
s(?â¿âT'nâlq¿ê3âààU¿å8Yã¡$¨¿îa¡Û‡{¿ïÿCÂw‰NOTHERunk3FGL J1855.6+0753NVSS J185612+075340?¦n£7Óß0?¸dŠä‹î?î™̂Â
?¸dŠä‹î?«úï5'5?À¨þõÀ3X?î@_ñ¦Ý?À¨þõÀ3X?Ðè¼­T?´.Òӓ~×?çõ‹À!©V?´.Òӓ~×?"'<«ÿßr?'~åå›~?ï[n ?'~åå›~4FGL J1857.6+0212¿àüÐ,[¿ØÛaåùÀ7••žÀ9oAÿ~ÐÀ@p7ÿÛ=@7ïZ–O?¸#¾5y?Ö½"થ0@ ¼cñA \?úv8kX?ïʙ쥰¿ß4È<V¿âùÁÍjW¿éöå¿âÙ¿ïÌn"rp¶¿ïЌ­OTHERspp2FGL J1857.6+0211SNR G035.6-00.4?°{Ý÷?Íaò^#î?íð]Ä_Â?Íaò^#ï?l7ÏH¯Q?{£³EWñØ?ïãÈ0·èP?{£³EWñ×?i¢ÒXî?Ý"£Qt"?ïŠYt¶Ÿñ?Ý"£Qt">÷¾[Õ®P!>ï`ç;	?ïÿЃHT¤>ï`ç;	4FGL J1857.7+0246e¿h¸.B˜°s¿Âÿƒ
6À7ô'|À9¡v¯‰Æ@ ê¿É.1Â@ü,9
ä?§!\=ú×?h'"èl?È2<Tì?ý‹ÐÓŠT¿ïàsÞ-è?ïÿàU?Íu¿æ=^ä'å¿å'$óÅ¿à™[á}3¿×²í'¶'OTHERPWNHESS J1857+026?âV3%%(Q?Ñ®Ó`hm?ÛS™µµ¯^?Ñ®Ó`hm?ä´îò7Tm?Øg¿ÈrÑ?֖"'W'?Øg¿ÈrÑ?⃔(/Ô+?¾¬
Kx³±?Úøׯ Wª?¾¬
Kx³±?àÆ(eʀ"?ǜù~áÐ?Þs¯4jþø?ǜù~áÐ4FGL J1858.3+0209¿ÞˆSDV|¿áu"@òŽ}À8øéëÀ9ûïº7žÓ@!ÅÈC¦@¤ßÎ1PÛ?Ùc²ó?­çÄgB?äÏñå‹	´?û3r@9V
¿ï™L'9«?ë|vÕIs?íœ&¨«¿á1J$ç@¿æóé;˜\ƒ¿ïú 9påOTHERsppSNR G035.6-00.4?ÓWpéiã?ÑÇÈp+Ç?æTG¿K?ÑÇÈp+Ç?ä5#\¬P?Øp:—Ú'"?ו¹F§É`?Øp:—Ú'"?à\ì-Uì?Á3ùÈÍ,?ÞßF'¥T)?Á3ùÈÍ,?ßéÂWñ¡?dž†ËÁ?àÔ/y?dž†ËÁ4FGL J1900.8+0118¿ê#O»E¿÷ìqþJÀ9'J HÀ:HgÒw0¹@òÉÞ/ö"@f?šIÂÂ?Ñ£#=­?Üû=£z@Ͼ¹ä'¼?þïSZ'É¿¡…¡êöÙf¿«ŒÂƎš¿ä¦ˆ*¿ìÁÓ_
+¸¿ìšƒ¿<ÁQ¿ïğá§OOTHERunkNVSS J190146+011301?¯Ódg½b?Àt´\U,?î²É¹"*?Àt´\U,?Лê;K"‰?ћxJ¦æ©?ç²
âZ5º?ћxJ¦æ©?½{'\CW?©Ø}WîÅÔ?ìP›w•?©Ø}WîÅÓ?—žÁ`­Pî?…| -i?ïC	ôú•y?…| -i4FGL J1902.8+1451¿î.ï°¸3@	&A³)À:l*pìÒÀ;½—Õt;@ cȑª@Œ$ÞܙÉ?ÇÕ{]2?[Ä}Y-T?ª!Þ:ø@|šCã…?îb÷ç,Êc¿ê»ëýê|¿ÜÔ	­þ«¿à@ï´XaÁ¿à'ààUÚ¿çt¨+,ÔOTHERunk1RXS J190249.1+145133?ïÅ×2䊥?wv"V>ó?}fº­\?wv"V>ò?ïðKšØˆK?'åCätã?_hÊNïjH?'åCätå?îðyŸ;jd?—O¥—ž‡? øfIY»?—O¥—ž…?ï§2ÓÖô?r®ÍüK4?†3K
{Bç?r®ÍüK44FGL J1903.8+0531?v'Ùè«Ñ2¿ÏPŒŠgwˆÀ8P*|«LJÀ:ešŽŒ@ØéH-–;@Ù7fžšŠ?Àä8yC7ã?ËQäç ¹@ã\[J©@˜/…)?ïkV/Ž?×!¦BõH¿çÄM¢J¿ç5†_*2¿èa.ÿÿe¿ê¹'Ñ!EOTHERsppSNR G039.2-00.3?ƒÎ·ÝÇ?©'eû$Zš?ï°Å# ˆä?©'eû$Zš?¤¤"Œc?¸À
X?îµ·Ç9Ç?¸À
X?Ãg¬H[܇?¯À@_³Œ?ë&íéß?¯À@_³Œ?›êÒwƬ?‹gpVUØÔ?ï ©lGYË?‹gpVUØÔ4FGL J1906.2+0631¿íG¬l¸
¿ÓVŠüñ}À9½1NV¥À:JNÇä/À@%ž©xß»@˦"c§o?ÔSs¯ûî?å©Ë@Ó@;ŽK‡½Ï?þ‡ýÈI¿Æ(!\F'¿ë¾aÔU¿ØÈç$'Ú³¿í!Äuæ6¿ïÿø="ßE?ïÿ /ÄêOTHERsppSNR G040.5-00.5?ÍÖÝ[ÈVT?Ðö|€" ?èŠH©
êj?Ðö|€" ?Ù*ó-¯\?Ö|9ö|ô
?ãj†ip(R?Ö|9ö|ô
?ϤOhþ2?´~3µÙ?è:Vì%Às?´~3µÙ?¥Þ1˜ª‡º?œ­Èá‹?î¢æuW"?œ­Èá‹4FGL J1907.6+0703¿ïC
Ô´hÓ¿ÖÑ#^))À8Õi´Ï€À:ÿ¼ä!}@!L/å¾@—ºÇç‹?÷ØÎbÏ1?»LemaØ?øæbÕ¸-Ù@<‰Ên£¢¿ïÿÆ¿l'ú?ïÿþR€ÖT¿ê¢ç@k€¿æ¶a@aÄì¿é0Ձ¥‡¿ß7Cõ"VOTHERsnr3C 397?Ìß霑(F?Ðè«Efý?èȘ۵î?Ðè«Efý?ÐâT
Þl?Ô­hÓôñB?çŽÕúýË?Ô­hÓôñB?؟à[æ?¿ZÃ;Y?ã°Ò¿y?¿ZÃ;Y?Ööåk±?Ëu'×?䄍1J'1?Ëu'Ø4FGL J1908.6+0915e?äñ(w3i?ۆAãz8UÀ8='ùCM]À9ÿ_tڝp@ IË%,à@$Hdà?àë¤Éx"v?Ҁ3â/µz@¼`ˆÖÓ·?ýCƒÃ˜þ?ïÒ7y…¿ádƒ7W…"¿äLg¢%¯<¿æ¢_I¿é ÃÄæN?­[ƒIBŒOTHERsppSNR G042.8+00.6?¼ÁH!ݺË?Á6¥9ž?ìgÖûÄH¦?Á6¥9ž?À²Z¿'A?ÉÐ$>¹¦Ã?ëÓiPoº?ÉÐ$>¹¦Ã?ÉWŸçyÿ#?±bÝ++‡?éª!€7?±bÝ++‡?¢±3ÝUX?—òGD(?îÔîŒÂ*«?—òGD(4FGL J1910.8+2856¿Ò	*n0Ÿ@!ͦÅÒÈÀ:_:Ôd¬À<H>¼(@!w×Å#`,?ú+RÿTÿ?ÅÛìdí•o?Áq¤ƒ³ÿ?û°^òԞR@©…—Ùûß?ïøøo"¿í¦÷P.½?ÏI5¾}ԗ¿Ôÿ©ƒq¿×kr¿»l¿Õ/â{ŠºÚOTHERunk3FGL J1910.8+2855NVSS J191052+285621?ïþqR)Ìø?)oF…g‡?(êÝc0}…?)oF…g\?ïù­þ‰"¤?g"ݵ¡W8?IHÛusq?g"ݵ¡W6?ïíX¹ùKD?jb§îb?b§F´»ò?jb§î_?ïíë·Ã€V?PYîøÜÏç?bH<©ï?PYîøÜÏæ4FGL J1910.8-6001¿î‹JáÀJAÀ9¢È:£jÀ:UàñFÿ™À<¸6<Òï@/H—H†'?ÿÍÃ7!Õ=?Á¯þµÓ?àݰʹ@œb^™éK?÷Ø腏÷?ïôºâ"Š;?Û:`¤¬¿ÞI
DâG¿å¾å¹,ÜØ¿ð?ïŸJžê	OTHERglc3FGL J1910.7-6000NGC 6752? §ø}âJ?§ãבeû?îõ€w!Û?§ãבeü?©ÿ½
qo?¾
Ç]&S?î`.(é?¾
Ç]&S?¯è¯‡ý=?£€`Cÿ?î~u€,?£€`Cý?'n-èsG?"¹ ÌÆÇ?ït¼f?"¹ ÌÆÇ4FGL J1911.0+0905?çÔ Úà9¸¿ÆŠæ¸Ü*
À6¦»¡+^SÀ9©\¥"›@ \Y(eNä@þš9҉¥?œŽ÷Õ9Õ?¾f{µ*Ó@#,Ùb…U@Y–8¼?ä²Àü§†?ì@֟^'¿àó\îî_Å¿âYöKKWí¿æ•V©Zý¿ã\νgÔûOTHERsnr3FGL J1910.9+0906W 49B?Ò…u»"¾?¦º¯¹?ïykÔR#Z?¦º¯º?\s½"Ar?g\~þñÛ?ïñÆ!6_G?g\~þñÛ?áFeŽÙ'?¸ YɊ |?Ýûs4âLÝ?¸ YɊ |?™ÈÂb^?;†Ìæ%?ïÿ"¥˜Üö?;†Ìæ%4FGL J1911.7+1014c?íèKg6:ú?ʑb}ù€	À9"¤ÏWÁˆÀ:C_?*¸:@öÐÑê@ÖÐ& û?ÓéLçvÇ?ÛÊދ?@
¨d©ÍÄ@z|rí2?¹¨w­áz.¿ärÑCT§¿çò›Þ˜QE¿çè§ü2ì¿ïÿàè@?ïí—䱛OTHERunkNVSS J191157+1007208?Ý	ù³ˆf?Òu"kêP"?á{&w»Í?Òu"kêP"?àA˵d?׋Y¿Jö ?ß|h•çé7?׋Y¿Jö ?ÓYµÆˆ°?µJ¡îCqT?æS%ž»¨?µJ¡îCqT?Èq:|
?¶Ö\|î?éã±`ú|¿?¶Ö\|î4FGL J1914.5+1107c?º¸×ä–ç'?r;éàåЭÀ8þ~Ä+=›À:mܺ€™î@Ú¹w/Œ`@¯P]¥?Ëô²YƒÿÔ?ØN»{ì‹@D7£~ö?úi#͏•_?ï¢á ÁÁ¿ëtŸ¢G¿âñ—‡p¢¿å߂ç¦lç¿ïêX~FVü¿ïu üÏÊOTHERunkIRAS 19117+1107%?¯Dç߇ST?½åsìˆ?î±'ŠË?½åsìˆ?³QG	ñ?Áx'&F?í•Ý—Â?Áx'&F?¹¹¾â¸ø?¯{òTÓò?ìÈÈ#¨üÁ?¯{òTÓð?{cB®nà)?e¡µÓÔçº?ïÉ9z£"??e¡µÓÔçº4FGL J1916.3+1108¿½Y µ•¿×ã	
¦¢À8hjª˜Å^À:#ˆY@û®a§»@$,<žìÀ?Â}BJþ+?Ï©ãhőD@€aº/;@£ -²k¿æprÄBº?ïÎ<~`ƒ#¿äyh6J>è¿ê×0h}—Û¿ì/#¿!é_¿æ=\aª¿ÝOTHERspp3FGL J1915.9+1112SNR G045.7-00.4?‹ä¤ã{?±Y"6Ô¾T?ïo·­ls?±Y"6Ô¾T?œúW^»Š®?±WÍ-c—?ï-E
#ª?±WÍ-c–? y"P–y?'–xj<q?îømÚöŸØ?'–xj<q?˜y%Çß.Ë?*È&«^?ï<6ÑÁ‰?*È&«^4FGL J1917.0+2245?ì0g>!¡æ@v®b~zYÀ:Rß&k¤"À;›%d=—:@îƉ;Ók@"%kÊSv?ƇE¯Ç?Š²?‹cÔn?Í©Ä_Z@ÁÛÍEÄ?ïÇSó¿ãt;Áw.5¿ì¶À5¯å¿ØýŸ˜¿ák¬N"r¿ïÿï0l¯OTHERunk1RXS J191710.2+224852?ïíøL·ˆã?dLßözçð?b³Hw?dLßözçí?ïú)±jYß?gÔïs°Êâ?GY:V˜€³?gÔïs°Êá?îûb~óÆF?—æy£°'¦? IØÛ¦?—æy£°'¦?ïßSزA0?^Ý0Ɔ?pV¦ßgò?^Ý0ƅ4FGL J1918.0+0331?Ãö
tü5íÀ-ÕM¤ÎÀ:Tâó¾ýÀ<jì$·@"*ÂsW‹?øé¥e¶š?Ècêá	ðš?Èî ÝÓN@B='1Æ@Ýw"áú?ïÄ:Âs­w¿ë
Шú_­¿Çè´ÊL"Ù¿Émêi?à¿Ò€XÀ`'Í¿Ü'kÏOOTHERunkNVSS J191803+033032?ïö"þ×J°?SÍlö:^?RØQjŸ0?SÍlö:g?ïüÀߦ¾Ï?[¯›¥€"S?9ùÊ	Žû?[¯›¥€"X?ïqPpxÍ?ÄGaÙÖp?'Õñðæ];?ÄGaÙÖs?ïÕrCÂð'?eÊLI—»?uFÞ‡¶ã?eÊLI—¼4FGL J1918.1+1215c¿îúd">¡¿Ð?ºà¼ôÀ8½3€`°À:HKjaž@!"å]<@¶"}æO?ÊJ¯;At"?ÝЌÀ\¾@±JÓbé@ ,|_Ìï¿àÓí½Þ€¿âzüö`D¿ä'§èM‡¿ílzFíû¿ïúÍ%¸ m?ïGnß0҆OTHERsppSNR G046.8-00.3-?Å«R5çÝ?È45¢–PÆ?ê•+zò†?È45¢–PÅ?ÇÓ©'KÀ‹?ЀþåB(µ?êŸmÝ?ЀþåB(µ?¸íÈKÆ??¥%áI
úí?ìâFÿ‡8?¥%áI
úï?šÒ\³
Wð?cC/YÒ?ï)mg­A?cC/YÒ4FGL J1920.8+0418¿èzžkåç$À>ˆXÿu—À9¨" [TºÀ;"×I''?@wì…#ëÃ@]ô!¥l6?ÍM›ê+ØK?ѳ]û]ÙÐ@7ã#Pg!?ý·ö|b?î€m®YD??ÛobäPÌ÷¿ÛÏ|'l+¿ãÿÜđ•¿ë	FОé¿ïÿ n4'OTHERunkTXS 1918+042?ÛSÿUv
?ÉN¾S}',?âVsUDü?ÉN¾S}'-?ÞÇð»ó¨?Ô.ÜÂÄhÁ?àœ·¢-?Ô.ÜÂÄhÁ?ؘSáÏÅ?·ëŁ+fþ?ã³Ö~?·ëŁ+fþ?з=%?"É?¬Ú6çhâ?ç¤am`=œ?¬Ú6çhâ4FGL J1920.9+1408?ÄRßß8?¢åŽå‹ŠÀ7ü֋'oÚÀ9¹°xÙ/²@µgJ0@'³Ù¶À?Ãe7'>?ÏxJAÃ@§~^ª°?õÉå"nâa¿×ÏVˁ?ïœ}^Ðoï¿èÉ5~'ñ¿é&$ÂW(¿ï9Ä6%¿å‹‰ $¸œOTHERunk2MASS J19210164+141003?'˳^b©?¶º[}O¡?ïi¢eï+?¶º[}O¡?†[q'îì?šz³ˆœ\0?煉î;`D?šz³ˆœ\0?ÂX‰7ÜÕ¤?®m,¤ð#ã?ëiݲʘ?®m,¤ð#á?<ÍbʶÉ?1†ï½ÕÒP?ïüfP¦©?1†ï½ÕÒP4FGL J1923.2+1408e?Ú)h'Œ·¿ÝŠâ²_¤À5âœáL¶'À9t3poÔ¤@:'-ºM@Z}Sèµ?'d—·Ë?»V%¦'¶(@'•Râûã@É¡
&I–?ïåæä¦f¿ÌŽ¢…%™B¿á'r½Œ¾¿â'¿Asè°¿æ²*ŠF¿å[1Ÿ4c4OTHERSNR3FGL J1923.2+1408eW 51C?ÉäKڏ0Þ?Èåå\(‹Á?é†í	\3É?Èåå\(‹Á?mrà:w«ö?¢«lL_â?ïâňT?¢«lL_â?æéùÁôÖÈ?³SèJâØ?Ò,|Rr?³SèJâØ?º'¬ÒÙ?|O@a'ë?ïÿj+ê™h?|O@a'ë4FGL J1925.1+1707¿½øpLñi?á†e_UPÀ9!<MŽ(LÀ:"*—ƒ>ä@ Úº¶ö@®÷ÝÏi?ó"»äG=?Æ꛿¹"à@®Ñ9C?òÕO[2¿ë"²Dx«?ïú|"eZ£¿ää­ßKÕl¿ç–Pn­\Å¿êäÞÚ4"¿æZêg‡OTHERunkMG2 J192501+1727?¿©·ð£³?Ä@^îÞ²Í?ì
É뉞?Ä@^îÞ²Í?­É¤0_ëT?½|Ǥ?î#e¼úK?½|Ǥ?ÓDÓ´ñ=?·g¼*&?æ]ø–%‡a?·g¼*&?¡I	½àÑ?¢Ò¤†‰E?îëooô!ó?¢Ò¤†‰E4FGL J1925.3+3705?ê	UÙ|ò@#™·|¯ÞÀ;CØ>ð֗À<¹šû@ Œ6%«á?ÿ1ž½c£?зObïœ?¹Ÿï^V?ðRtý¾@àDª~ï?ïÿÅbu@¿ã+ÂüirŠ¿â`GÓÔ(¿äG@'‰?È=Qӟ$¿ïþæZ<ŒxOTHERunk1RXS J192520.1+370527?ïÿ×pB>õá^0"Ô>ôGõ^ò³>>õá^0"?ïü,²V¼?`%˜@Wü/?>šmJ²?`%˜@Wü0?ïåe»ÿj?t1ĕ–9?júšD•Q?t1ĕ–;?ïü®Ös?1Éyü]¨?:‰LgoÇ4?1Éyü]¨4FGL J1926.7+3027?ÝR™¹~@¹èÄzÀ:•ùµc$À<UÛÔ§@xY W¹O@=áâß?Ô.ËÅeÐ>?ç|}T¨@LлnÖw@Ë#ˆÆ7²?ïý± žÛù¿à¬^YQ«¿é!¨üãëͿ웭p3T¿ï÷7ÿöšÑ¿ïôUªV€OTHERsppSNR G065.3+05.7?×Ç!rO?Ïtš%¢¿?ä}ïFØ9?Ïtš%¢À?ÂÆOÍ®Ts?É®üQŸ#f?ëNl"jâ?É®üQŸ#f?ÚÔ#¤µ×?¶æÚZN³?â•øî-¥?¶æÚZN³?®À(qq?"¬Ì¢o|l?îƒýxèð?"¬Ì¢o|l4FGL J1927.5+0154?ޖù^+ôÀèp—AÑÀ:Ê]†ÃÔÀ<-/à˜[¬@!ÞÓč¹?÷êSá(¤d?ÓûÒß5…?Í6ðÂuZö?ý[íœP-?@d¾Ö"÷ž¿ïǐÀI‡?ïuEâb`G¿àkbŸ1‰¿»<
rIÉx¿ØmÙ8>¿Ö0Z»¸RlOTHERunkNVSS J192729+015353?ïòt•äì?`H0ËØ
?[ÕÐ6'ö?`H0ËØ?ïùt¹v¾?~8–rt?J-'Ñf?~8–rt?ïh÷/š`¼?>B?Ž?'á³èh?>B?Œ?ïÚèéÉ_š?dtµ°¦?r‹‹P3
?dtµ°£4FGL J1928.4+1801c¿î¥±I¾Õ?ÒC.=€6À8½ŽwýhÀ:dÍcˁs@Pœ¹ʪ@>¤€}há?˔VúËë?ŀ¬"]M
@[µƒ+ß?þÏðH'2¿ï˜"}?ïÿÍgý?¿êpÓ§²a¿åÇ~)¿îÝ¡0fÐ?Ý»4‰tˆhOTHERunkMG2 J192830+17598?¿ÅJäìV‰?ÃÀü†÷£?ìV£bu/?ÃÀü†÷£?·G`*ZbP?ÅI§‹ÓÎê?íú´³¶?ÅI§‹ÓÎê?Ó0(­í?µ&ºLä…ì?æ~gë©	?µ&ºLä…ì?Àyð¹?³Õ7'f×?ëøaƒüœ?³Õ7'fØ4FGL J1928.8+3126¿âòZ	IP@B÷+E((À:g²Û‰þòÀ;ë×!ºdë@Ô]ú@6?<Uñ¤?ÌÖ¬	2ٜ?½FÚ@9U?õŸf²¼€N@ðHäJlá?ïÿâ£Î¦Â¿ÐP¼{Eñ|¿íåmã2ià¿Ë'yꧩ'¿æ"9Pƒ¦¿ïÿ¸8º1OTHERsppSNR G065.3+05.7?ïÛJï[?zLږ†?rZ¿R?zLږ†?í&p@zD?ÁïqÌÒYÝ?¶Ì}ü/mç?ÁïqÌÒYÝ?íú2#ÔÂ?¡gæé=	?°.nç)Yô?¡gæé=
?î=Ä¥`Z?˜Gù&ª_?®#µ©úZ?˜Gù&ª_4FGL J1929.8+1832¿îFVdJÏå?Ð=çâQï6À9i>‡ûÀ:x¦'@âdc¬Î@µ€šÅÄ?ù.¤"‰—Ä?Óf|`Ρä@`µ$9›,?ößz!8?îÐ^½$¹¿ëç?¿³‰°¿rÜHÚ~*¿çz
½É#˿胦³]þ¿Ôòb~OTHERunk1RXS J193012.1+183201?͓ÚU²×?Êír'[šŽ?è›	j"~Ë?Êír'[šŽ?јá¬Õd?Ô~?&…!6?ç3ò)•O?Ô~?&…!6?ÒÍÈèc‹?¸°}¾S
??æû™‹Î:?¸°}¾S
>?°ñþ"óä:?¶§ÅúHä?íáÀ/aƒy?¶§ÅúHä4FGL J1934.3+1859¿ÔÞ÷‹Ó׿Ýó‡·aÀ8̔<b†ÞÀ:lþÀdß~@s	%˜•ä@¦b…0V	?Éлļ³?Ớua«í@¦Ó0"'@ÖJ¦Ar¼¿Ô€˜›¿äð˜ÿjÙ¾¿ç/æw˜½Ò¿îvþdŠ¿×@Ъ§Þ׿ïÿôa¼2¡OTHERsppSNR G054.4-00.3?ÅĆèª?Éh¯.ÓU€?껎ÞEÕy?Éh¯.ÓU€?¾çÿµyòå?Ë
Ìd‹¨"?ì#	PÁ¤?Ë
Ìd‹¨"?іs¡Yƒ?ºgìŠá
f?ç4Æ/S>}?ºgìŠá
f?•êÆÀ\ô7?•m‡U—à?ïP©Éý^?•m‡U—à4FGL J1937.0+3003¿Ì/:®=YÎ@nJ82vuÀ:j´©ÀXÀ;®º××ÂÊ@ÌýÔ+»Æ@ƒπÜ3?Émõ¦à©ù?¼™:Ü?òŸ
纏?õù>ëM@{?ïþœÚñÔ¿Öz€5D…¿èў"•V>¿ì‹©¡¤ý¿ÙLªÓ}Àö¿Þþ®Ç(HOTHERsppSNR G065.2+05.7?ï®çžb?‡Ûœ÷pŽ?"Fxg~b?‡Ûœ÷pŽ?êˆ7¬g4w?Ë÷¿'È'ö?Åß!Nc.%?Ë÷¿'È'ö?ì_elؽ?§KñõÞ­?½ԙ:w?§KñõÞ­?éKy"¨Ã?³åv·§|?ÊÒí\ó¾?³åv·§|4FGL J1946.1+2436c¿Ø8"°üôg¿µê‡a¢v&À9ÖPfIàõÀ;1Cót×B@î«}œ¸Þ@ëø[ÆÐ4?Дr¾8Š`?ÛLÜõ)@¨>]2àþ@ìA‰ã>¿ïÿ…@ò
¤?ïü&âAþþ¿äIE=÷²T¿á‡n¾ú|3¿ïÿú Âî'?ê<—Ëc@AOTHERunkNVGRC J194625.5+243638 ?ã¶Á¦z{h?Ð*Cî[0¦?ؒ|³	1?Ð*Cî[0¦?੝÷]¯þ?ÖÿÑôë5o?Þ¬ÄD ?ÖÿÑôë5n?Ýèäśüñ?¹š$…ûU?፝2‡?¹š$…ûU?æn	¢?¼1§'ˆ4d?Ó×#íÃö¾?¼1§'ˆ4e4FGL J1947.7+2744?ãE '®"?òñBè²ÜaÀ9|Ô4 ½À;)}œ
`@¨MŽ(LO@NU:Ä÷ì?Á¸Û=ÓË?ÐÂi\ƒ@Ö,wWOr@ý%­c¥í?éìjVµï;¿áÛÌ`ëÓ¿Ùp_ùºÂ¿æïÄH™Í¿èGóÐG¿ïÿÈ¢› ÛOTHERpwnPWN G63.7+1.1?ºý›>җ?·U¥ó?ì®L˜%­?·U¥ó?Í5Üÿ€?¢?ÐxýZ®‰ù?貈Àð?ÐxýZ®‰ù?Ö<i¸'p2?µõÈü–=·?äáË#·Gç?µõÈü–=¸?Ô®T¡H
?­—#¸Å®?åû¨Õ¯[ú?­—#¸Å®4FGL J1952.8+2924¿ïPç'>hÚ?ðórS³À9‰"ç¨ñ%À;F"ÈŸ@£@iëw1æ@Hþƒ(?ÉçE³Z?é£opÑ#t@–¼b~?ü¯$¦}ƒ¿ë!ƒÞFqԿـaÉÁ¿Û"Êý¿³à¿ëÊ55kó¿é¥ŠÔø³¿ïüÚ±'ÝãOTHERspp3FGL J1951.6+2926SNR G065.7+01.2?zrÃuH
é? ŠqfÂ#?ïËyoä? ŠqfÂ#?¤ÕÁÝ3%?º'B.-sÁ?£â,Î?º'B.-sÁ?°˜zÛÐkª? >x¹Íâ?íìð¤…ò‹? >x¹Íâ?Žqì·Q"Œ?{Æ¡.ÐU?ï†8M"¹²?{Æ¡.ÐU4FGL J1953.6+1846?ïuÅò$ÌÅÀ)ùHUÚ'À:7ÁM<ɵÀ;Ë«¢°™@OÔS©Ë@ú37dñ?ÈÈZLQ½?Ҹ϶¤l@	ç™ÅXd?ýbG‹ÿ"?ïÿþÞ÷¿àiÒ+±^²¿ç©.ݎ$¿æ.52ôD¿ïÿõƒ¥;Ž¿å¡»§
›OTHERglcNGC 6838?ìI€Ê²€?¾Ò×®_òœ?½³ùªkÿÛ?¾Ò×®_òœ?âV÷Šg?ԇ9SBÂ8?ÚýÉRë0?ԇ9SBÂ8?ÜJፆ?·á‡‰Wj[?áüZò9<?·á‡‰Wj[?Î)Ö•ÿ?­iíAƕ?èuŠڀ9?­iíAƕ4FGL J1955.1+3321?î Ìó¼@WŸß-øaÀ9ë!Ð4`ZÀ;U]"̃@6¬'=@o ×{|x?ȉº¾ØBw?ÔE,¥$'1@
yyh¡ª@	S§t£•ò¿æ±Q±£{›¿æxlâÿi¿â!?èÅQ¿å§ŸVqý¿è°ù'7}E¿ïÿýFKêOTHERsppSNR G069.0+02.7?ípäCÂL?´`'ÛĜº?´xÝãí¢?´`'ÛĜº?ë¿È^ëú?͔ÿ¿ßÀ?ÁއôP?͔ÿ¿ßÀ?è™Ö´å"?°ïˆp@èw?ω˜¥,ið?°ïˆp@èw?í³¨NÆ	? 
3qÿÙõ?²b½‰Ï·h? 
3qÿÙõ4FGL J1958.5+3512¿ãÖ¬Â0j@J蹒]eÀ9ÀmzVÞ3À;"ëü<üá@ p8Zdz~@9{Kй?¼vY£Š^?smóÔ#?¿¹¶š†T@2õ«hN?ï<ÌQ#ß¿Ýüê6jY¿ãí÷¿¿ž¿Ú¿
|?k¦¿å"}¾Ùû¿Öh,#Ê_ŠOTHERhmbCyg X-1?ïÔUûMÚ?s})rLõ[?uÕY2ú?s})rLõY?ïö½Ænão?r¥á1´?R"s"9$W?r¥á1´?ïbPñY'?‰4–t ‹?Œ'ké›W?‰4–t Ž?ï«1C<b¢?q€v¡©2?…3¯0çWš?q€v¡©34FGL J2002.3+3246?êr§úgLº?ñL] l‡À9u_€™"À:Ò;ߪ#@
+YuO@A\Á¡ö_?Â(ü8V2¿…®Ô5Ä)ˆ?Ãjt "?ði!#¼Ñ?é9Ÿ=Èb…¿ÞD­à#¿èær@U¿ê‹¼[f¿áª‰ O«º¿ß<À»ŸnOTHERsppSNR G069.7+01.0?í8¹†Z6Ã?¸ûÚ&ïl?¶:3Í.Iø?¸ûÚ&ïl?êhª7aƒ ?Ñ"ŽÇ"?Æ]W"yñ€?Ñ"ŽÇ"?ëT|ãâ˜?°…)×Èä<?Ãú®pu£?°…)×Èä<?å"bSç>Ò?¶{•øÝK?ÔÙ;X1'\?¶{•øÝK4FGL J2004.1+2517?眾RÔ;_À	ÓAü#ÒmÀ:}–FþÂÀ;0ñ9" @–—G"ÎÜ@ °«.?Ô5Ä<ÛR¢?à¯/˜sÿ¬@	)5ƒo‹©?ÿê5mË	©?ïÈ8éU™?îM]®±Ú¿á‡ÜmSÀq¿è¿ø¨ó©°¿ïÿáa¯G?îRý"ªúÀOTHERunkB2 2002+25?á‰Ì¼C"Â?ϒ"?Üìf‡xÖ}?ϒ"?ã<ÜeJ}?ÕZ2Q³¶?نG4åk?ÕZ2Q³¶?Øjm'è?»"OĜgÑ?ãøÊÉló?»"OĜgÐ?ÐÖüÀØ/?¹á½¶ýyÚ?甁Ÿ"ðh?¹á½¶ýyÚ4FGL J2004.3+3339?ƒŒE•û?ó#5#Î;bÀ82(1wqQÀ:'µÜÆ?@¨=ý;ª{@v½+o"?¬ Jžðת?{Èù-©@"ßGù"Õ@&†pG?í%^>#Ò¿ÔM€flÆ¿Þ®<Sme^¿ä?'Q¦»Á¿ê;Á!Gù¿ä«¢æIu•OTHERunk3FGL J2004.4+3338B2 2002+33?¦Æiy¶?«Å«¡¦?ndž?«Å«¡¦?¡¥²áj±®?·t@ÏC?îå¤ÑéTå?·t@ÏC?ÙOiÌT,ì?µõoÙ6ƒ?ãXKÕé‰?µõoÙ6'?©²}Y¿=?ŽÕ¢Y1‰?îdØ*d|?ŽÕ¢Y1‰4FGL J2013.5+3613?š¢IæË?ðDq´xB1À9D5®7¶PÀ:ØÇNފd@È´p_Ž†@êC5öI?Ą‰bÙ?×Ò( °y°@zÒÁÙSÄ?øÅPt6³›¿çF3k¿Ø·Œž´`š¿á3€?ÖY¾¿çòøp¶L¿ì¯ú..ç¿ÚgzÍüwµOTHERspp3FGL J2014.4+3606SNR G073.9+00.9?–'Ì0â¯%?¥xßììçæ?ïKqžxê‡?¥xßììçæ?Ȍ΀Y{à?Ï ™yp·?éÜÌ_é¡?Ï ™yp·?¼ÐU[ìeÄ?ªW}´¾—†?ìeõT'sH?ªW}´¾—†?Å[²ð®?¦:¬Jºj'?ê¾¼éCÕ?¦:¬Jºj4FGL J2016.2+3712?í+Yƒ)~?ñÝݖH¬AÀ9+RFòÀ:Syú—á@"5g+Þ*B@—|ˆç›?äßzÿ¥' ¿©ƒ—àÃ
?ô« b
·?ýRAüNŋ¿ÝGµ¡7?ï-.Â
Q¿ë€#¦Î5ƒ¿ãÛù%k¼¿ãKêN½Ó5¿ÜsZÀ•ÝOTHERsnrVER J2016+372?ډQp	ÌË?ÓQx6?â»WGûš?ÓQx6?ÞC4z ¥?؆VDÒ?àÀ^eÂï®?؆VDÒ?ãÐw‡#€?ºô³wœH«?Ø_àñ¸þ?ºô³wœH¬?äf}¦¥
?Äq¯¹víS?×3ã²µå?Äq¯¹víS4FGL J2016.3+4953¿ç.mŠ§@ ;EkD¹À:²€	¥›0À<`
šó5í@!èÀA¤?ø^h5sT?Îë``½Û?ÊO'åJr?üôÙáˆE´@XÛ¾­$f?ïðKAœØh?ïÿQ"W6?δ°¨©Ø¿Þ'Í»à¿È%6Æ:·a¿áБb"sOTHERunkNVSS J201619+495324?ïò9GŠÈ»?b:ó½.~Z?[pênˆ6?b:ó½.~X?ïéíhH?…v¥?f—á·îæ?…v¥?ïwdiú[?ÂV=Õ¢?'~'À´?ÂV=Õ¥?ïk(Ò÷mÓ?"øJ&%Ü?'šå¡E?"øJ&%Ü4FGL J2021.0+4031e¿î"‡!åÕd@'âûã:ÍÀ6ûî'):ŒÀ9ºG²F8É@!ë$ ?ýþ«×‰¿1?¦ÙÞÃð/?¯BþñüÌ@Dnœ•Í\?ö}X@?ëIÒF‰QM¿êPãèrDÁ¿åŸ£i&4G¿×Mn]UƆ¿ÜºQ,k¿ßŠoŊ¹,OTHERSNR3FGL J2021.0+4031egamma Cygni?å¡þÄ{u?͋Î:põ)?Ô¼w÷	?͋Î:põ*?µÏ¦ÉVÏ?ÊVbí(¬'?íF&Õ=‡?ÊVbí(¬"?ås4"@?µÈw,§Í?Õі×ß?µÈw,§Í?¥<üMú?šà5"™0?î¬?@;/ ?šà5"™04FGL J2024.0+3202¿éÚ|ΏÿÅÀ	,ºËCÀ9Þ Ž€`ãÀ;GµöâJ@ {¼ý@Á…pí©?ÈÚþ=Þ?¹E\U–_}?ö8N%'ö@"I­/?ïåÑ0é­?ʄ‰§‰r¿ä™þ³ú™¿è'9
gǏ¿Ì†£V‹}¿ïÿ¶ßO±COTHERunkMG2 J202410+3203?ïðb,ÿNƒ?_UžÒ|Ý?_;¦búq?_UžÒ|ã?ïö0t¸j?~­èò
?SŸã*ø?~­èò
Œ?îg‹ìX¦-?Ÿ@kVÐE?©‡A:u"?Ÿ@kVÐD?ï_둀Á?‡²¥!TIí?"Ïçß?‡²¥!TIí4FGL J2026.5+3718c?å¿\+
–¿àЧLàƒcÀ9½Í!†b…À:ßöX·Q;@ÔÉEƒÃ@¥
ÙwÕú?Õvzۓd ?èfÃî×¹@
me¼{a?õ°r‹ã£~¿äsþÔV"¿èªý¤Ûìû¿Ü`wIJ¡þ¿îø‡›jT2¿¾_~8j*¿Û•Ü
Wq×OTHERunkNVSS J202726+372249,?á |.¿ð?Ҍ«û6
£?Ü¿¢€Þ#?Ҍ«û6
£?Ý䊵åì?×hôv±a?á
º¥
)?×hôv±a?Öðâ)(UŠ?»ôaƒð?䇎ëkÕ;?»ôaƒð?½:ìªÁ'?¹`'œÚ?ìX¢j§ÜN?¹`'œÙ4FGL J2027.0+3343¿Ü´=ŸÍÀ8''
À:u¹Èä
À;…-RH¢0@#±"™ªŒ?ýgQbÉ"ô?ÅcrÁ¯Z¿®—Azž¬©?ð'¹M"‰?ú'Ÿµ<O¿îy`^dL?ïÚ­`ûH¿ì%V¿ÝÀ>Æå,¿àQù\wпá6—Á¨+ƒOTHERunk1RXS J202658.5+334253?ïï"× Õ?a|uæÌ5?`{è(ß*Ì?a|uæÌ6?ëÔQr'å[?Ï_Á~?À®º7`j–?Ï_Á~?îzÅþÑ`?·JWӖ?¨S éÿÃ?·JWӕ?ê–Dw-/?ºÿ™¼?ŧÒî#KG?ºÿ™¼4FGL J2028.6+4110e¿ß<ÂÞ
Ë?öW¾VèDÀ4–š9ŸÀ8¼ C@ZgPœ$¹@wkcü(Û?…kŒ.æ·? ¹L^ʳ@¶Ã ¢@wu2)ô?ß&2dZ™¿Ê¼˜·œcù¿áÔ<iÌ¿á¹n¡q€¿âqPÚãæſޏ¹OTHERSFR3FGL J2028.6+4110eCygnus X?Ô¥çƒ%J?Õ·µ
ï#ö?å­>m[?Õ·µ
ï#ö?½1ì™ÿÎå?јUqAA?ìYÂlÀ#?јUqAA?èj—ß?<º?±9ÑÛ?ÎU ƒ
?±9ÑÛ?wŒöyKZ?oï<¥®Ó?ïÐæË
i?oï<¥®Ò4FGL J2032.6+4053¿Ò¯E'ó˼?äO\"UŒúÀ8ÉRÄÈòÀ9ûtä®jâ@R
b""Š@´œU5¼?Łø4È?ÔNžÃO @óíx:¤@¨×Ðâ¿Ô(v;©Ï¿çIüm¤HI¿êêgèF¥×¿è–Ñ"qïÜ¿ëÀ©s+pÇ¿ïÇ/¿`R¦OTHERHMB2FGL J2032.1+4049Cyg X-3?îÙP("Z®?²i#>r;?¢jývÊU#?²i#>r;?å/ÅÐó5?×°¹>V)|?Õ t_Þ˜?×°¹>V)|?äÝ­~áJÝ?³ô}®I`?ÖD¥=jG?³ô}®I`?æëÎÁÑþ?½€•óÜ?Óô(b|\?½€•óÜ4FGL J2041.5+5554?µ,x¿m@ é$Jb#âÀ:Ù­äÀ</êp'@2=²hŸ@^´UªW?Ð?ÐDÑkB?ÌÔÜeÇ6?ýeuU²Ê?÷ …[Ÿ
¿Á³k¢Š?ïäÂAÉy¿çL`RP¿ÞCиò$¿á!Äuæ6*¿ïÿîÝÃÀ	OTHERunk1RXS J204129.4+555144?ïGŽ\Ý­?™_rr^³?—N4dJ^?™_rr^³?ç§
'²>T?Ï啂0ðß?б尛ƒX?Ï啂0ðß?ì½'Ÿ´p?¬'ÑÙé´¬?º[k\‡?¬'ÑÙé´­?åÖ0õE5ò?´.kú':<?ÔSžu"?´.kú':<4FGL J2043.1+4256c?âŒ&z•e?Ô[Ý¡[YîÀ9;αð¨À:i­°hé@¤S³Ü;@O¡»§
›?×¢‰G;ÿ?í~âÿ>9!@Xt »ÌÊ?ü»ÞDno¿æ›å¿ê¿ÖO© ø³…¿ë}Žc|¿îÛ-M@$³¿ïӘc8´|¿ïø~a.ïOTHERunk2FGL J2042.0+4252cNVSS J204232+425813!?å†@Ü©î?ÒÛ׺ü\¼?Ôó~F­È'?ÒÛ׺ü\¼?ÂÖѭͦs?Îó·]¦X/?ëJK"Œ–b?Îó·]¦X/?Ü5ÇØ·yx?·QÉBޗv?áå¤CD?·QÉBޗv?cȲW"çA?Szð½ðxˆ?ïì7M¨{?Szð½ðxˆ4FGL J2045.2+5026e?æí#ø
@®…bªðÀ6ÿp·ù1À:wÖåTƒ@¢¡Åâø³@8¿E$Í?rj֍•Õ?Ì&ãÚ˜Á@*è"úô'…@dk@?á?Ä/ZöñŽx¿ÖËF…¿å‰·~±áº¿çÏ°!Etÿ¿ïGšþôgF¿ïܛ¬™PžOTHERSNR3FGL J2045.2+5026eHB 21?eX,g›?hÀDˆß'?ïêÿ§Ó˜ç?hÀDˆß'?h?O6Þo?‡àaõÒÌî?ïçÀ°É!ä?‡àaõÒÌî?Äȯ6–?°Ê]`½UØ?êÍÔ;ºò[?°Ê]`½UØ>ê4½ÔâÑ>åÉ°ÿw€i?ïÿåËBû+>åÉ°ÿw€i4FGL J2051.0+3049e?ÑÞ­16hºÀ ìµ»8OÓÀ77Ú¼y˜rÀ:Õçd'ÇÅ@¡ÓÏËZ@ž¸Ø#B$?˜¾"ºêø?ÉpÐãõè@-f8Éu)x@ˆÇÕGj?ïÁ´ †å¿ÕL@ËLD¿âßhæsg¿åÛ¹™ê!q¿è*'ò"È¿ê†Iàô¡þOTHERSNR3FGL J2051.0+3040eCygnus Loop? ÍõèOh–?¤­¢uû?îó ¡{	w?¤­¢uû?r8í…Tp?€uy‰
èŠ?ïۏÞ$õW?€uy‰
è‹?Ù®"¿Ìé?¶0¦ë€â?ã(¹n ‹?¶0¦ë€ã>ꂖü˜N˜>ìTø™W?ïÿå}ig>ìTø™W4FGL J2056.4+4351c¿ï÷€ñþ¹°¿ïDË ¥<À8âô2}À:¦"%¼R@ºvQëÛ@ûB+»?Â)Zl] ?ÓÆ¢[Šk@!w~¼ž?ø-c­úN»?èáºÅc¿Òô&­é²·¿åá?(‰â¿ë	ë;LÝ¿êåB_ !¿ïÿÿ>¹úOTHERunk3FGL J2058.0+43471RXS J205549.4+435216$?¨3ìçàK?­Hoy;N?î|Á1ûO?­Hoy;N?Ã#E¼1¨u?Ì+?h{·?ë7.ó•ã?Ì+?h{·?²D¥ÕŒ'?¡Cu$×1?í·oËENn?¡Cu$×/?†…æ6&¶?q:lTv™ë?ï¥èg'gé?q:lTv™ë4FGL J2058.7+4454¿Üfž®$v¿âçF`6¡}À9t— Ÿ³À:þºoÒö²@«œÂ˜ìK@7á2µ^ò?ÐÔbãz
b?ÉH±õ…þ‡?û}E‹$‹Ñ@P	N][%?ì¡ÚƙØ?ÝjùÞ}Ï9¿æˆž¿É.2¿ç»Sþ"Õ½¿ïø*~XËs¿ï–ü0g¦ØOTHERsppSNR G085.9-00.6?êç§&5?Än2Õ?ǘcícg,?Än2Õ?ì&¨íÍèD?ÊuÌhST[?¾Ê¸'½ã?ÊuÌhST\?åþ]vÙ?¶Š—Øß¡¾?ÔÙEM?¶Š—Øß¡¾?êÌ_²h" ?ªòßò(0£?Ä΁6]í?ªòßò(0£4FGL J2059.7+4837?ä2J9ËLž?ûF8Éu)xÀ:º}SèµÀ<T«@‹
‹@ÝÌÃèw£@‰à¤&?ÔÔ@ƒþ¨?îh—c^t*@¼8zšÐÑ@ªæ:²œ¿ê`ª?.>,¿ÞHšu%F¿È¢]b†²â¿Þ¼£¿ïý²6ci¿ïºýÂcOTHERunk1RXS J210008.1+484122?ÛÉ"ç"Ì?Í9¿Õm
N?ây¶5š?Í9¿Õm
N?ºßž|`1ð?É Â&D?ì¤0sùÃ?É Â&D?Þ«®Êmœ?½}˜IÏ?àª(šÉ?2?½}˜IÏ?¯ Ó²Ñw?®}f;[z?ëTËK¢?®}f;[{4FGL J2123.9+5158?î"ÂW~—?óhG7À9ó¼¾aÐÀ;
cûRV@¢ì1l½@¡¬Âk?ÖzРìÊ?á›Ό@@@Þ$
%'@5òzÜ?1¿í|ñýþ?•·©=ë6ß¿Üàû㐳—¿éѺ¨¿ïûR}ÔA¿ïqNŒU
yOTHERsppSNR G094.0+01.0?¾uêÇCŸî?Á†°ÞÇøõ?ì1B§Œ?Á†°ÞÇøõ?Êg­šÅ,?ÐG—¥pW?éf™N¾5?ÐG—¥pW?È)IÕ?²ò*ci?éõ­¸»[Ë?²ò*ch?ØÒBq³¶?¹,uÞB¦?ã–Þ÷G&%?¹,uÞB¦4FGL J2129.9+1208¿ášSâ¿8(À;Q½aõ¾^À:1'"ªLÀ<5š5 Ë½@í§°³''@?"äMòÒ?È'amÙ!?Î!µz@OjCj¸Û@ï/1?¼§»rÈ¿âè
`+8é¿åo‹^¿¿ìò_c<æ:¿æoA×:å¿ïÿ»!(ĚOTHERglcNGC 7078?ïäù{§¾á?l™ÏÉÀîc?k"XA‡?l™ÏÉÀî_?ïúG'­¾ª?chÔSô?FãaIXl?chÔSô?î0§Â³C ?ž‹‹á­ÏO?¬õƒÔËÆ?ž‹‹á­ÏK?ï¶Dãâmž?m 5¤;¯?'nÇd˜ž?m 5¤;¯4FGL J2217.5+6346?ïæ`:ë4K@7hiÎÑÀ9Á²'ž«QÀ;ÆAÖd%D@!	ò«¨?ý顄I¦<?ʊ¾	w‡?Æ*"ÿ%À@I"¹`~@×èØñô$¿ï{ Ôvd?ïôx½«ò¿å/ù‰¿ÛõsŸ‰ó‰¿Ø§–ýˆ•¿ë?o¾ÁÇOTHERunk3FGL J2217.2+63461RXS J221728.9+634714?ï÷Í«³°&?Rðµlk…ò?Pd¨˜Ÿ³ñ?Rðµlk…ð?ïÜgfùH?"˜B@â:?qÌL÷ƒ\"?"˜B@â:?îI*p1? Ï_Ô?«m^üî?? Ï_Ô?ïVÿvՄ'?†øê?©?• %O{'?†øê?©4FGL J2219.5+4653¿í°)ÙiÀ ÙXS~,VÀ;W«p_À<ˆé¦!gY@ Á"ý}™´@ÇÄ\»Â¹?ÄÀ¼ؑ|¿«å'²¶?èåRŸà¸@œw!ŸŒù?ïþ~ö€$~?»Ä‰1l‰–¿éXޛ¬C¿ßêÙþ
·y¿ìŽ°Ëæ?åÄ #!OTHERunk1RXS J221919.9+465137?ïêÖُ,?g2r?e<i&pÓ²?g2t?ïóƒá.‰?y¶=ë®Ã7?Xùð=¢ío?y¶=ë®Ã7?ïb¿JâÇ3?ŽhtþE?"¨£§?ŽhtþC?2M䕠?rábg¾ÇJ?€Ûl†Ú˜?rábg¾ÇI4FGL J2241.9+5729?êY©K²Š¿ñÈ÷ŠæxoÀ:!´¢3œÀ;"¾â(@Ûé	ïB@ðæ[L?Ïfr»3rH?ËÙ©T!ÀD?øö
³¸)@¤[›(¿ïd~š9Ҋ?ïþÔò5<"¿èӐÁê¿çŒ>'Γ¿îò-Lie?Óª¿^UKOTHERunkNVSS J224154+572700?èƒvýsÅ?ǵg€+?Íò'¼
0î?ǵg€+?ìÞåìԍ'?ȶS!0½?¹Й["{?ȶS!0½?㾶)æ?¹Ñ²r'‹»?؂"ÁϬ1?¹Ñ²r'‹»?칚bÒ?¨§dDl?º3/ÿéi?¨§dDj4FGL J2254.9+5802?׎G>‹|¿ö…È̍íÀ9úùXF3À;œØ_¨D@çõ±óW¦@ål†;?Æ5Ÿôým?½ó"Uâá?÷rÉìG¼W@?7àÁ÷?ïÀ"¿óuƒ?ë§xª`¼¿åÄíz¹¿äM5<ø®Ó¿ê'`eŒ¿à_ô¯iåOTHERunk7C 2252+5740?ë%Tڍ™?¿™Gº]Ê?Ãïj¬•ÉŸ?¿™Gº]Ê?í}Ìö?Â䚂zÚ?´Ÿ`OR?Â䚂zÚ?ëk£îÝ?­O»Á¤km?ÂS³pD‰?­O»Á¤km?邓Jãý?©‡äÀþ0™?Éõ²ÔpÅ?©‡äÀþ0™4FGL J2258.6+5847c¿×.¥c³Ù¿îSíPÑÀ:<§Û{¼9À;ŒV=#vþ@ E)ØÁw¯@j[{PÙ6?ÔxžaÕ]?Æ0C>Ä?ñ¾Â³nVö?ñev&wä?Ä8AåӃö?äÅhT}0¿æµAjÙh¿ÜýI׺f™¿ëqáÄ«–¿Å!]Þ,›"OTHERsfrSh 2-1520?æ¸Ã{/AA?É%"®"LJ?Ҏy	¡}~?É%"®"LJ?çÅ[;úZÇ?Ó_í5²ï?ÐuIˆJs?Ó_í5²ï?çèlÚÀð?µ/#ôß?Ð/'ÊJ~ ?µ/#ôß?Õ¹n‹ž¤?µyœ¯ùs?å#Hº0ô®?µyœ¯ùs4FGL J2301.9+5855e¿çY§"2ò¿ðy`>.9À8¥ÞC¯'À;jÄ$"õ@ "öøogí?ÿµè"¹7Å?¬AÒ³@´¦?«"͏@'2úÿ?@WÚœ&¿ÔEìþñb-?êÓÌ@
>¿ÞU…2à'¿átA ´@¿ã3>)[n¿ÜÔ¢¯OTHERSNR3FGL J2301.2+5853CTB 109?ï:èB¯x ?–Ä–cÿë
?˜¢÷ªëÿ?–Ä–cÿë
?äíú1û¯?ÖèúÑÁ|?Ö$þ¢?ÖèúÑÁ|?ìÝJì	F?¬Ûq.½fõ?¹¯¸ŸµÐ?¬Ûq.½fõ?⥕þ†Aã?¿P6´·ÈØ?Ú´Ôó|7?¿P6´·ÈØ4FGL J2315.9+5955c¿ÒüáøØ_"¿èOQ‹N}À9V®ÃÍIÊÀ:öÕsd{«@b‡üŽ1@jî+¸ë?ÇΊ<."x?ÇõíÂæ™ý@˜ÿàöO}?øÀÛ­:`N?ïÿÝe¡D‰¿æØO·Î8¿ä»P£‡¿é2*õw¿êìóžGÔ*¿ÞŸ‡ÜôOTHERunk1RXS J231543.9+595510)?æl¬úÅ?É'^…Uo?Ó'æ¦
u?É'^…Uo?ägÈ;¬ š?Ôuo²\0?×0oˆ§¾Ë?Ôuo²\0?ã?äÓ!D?¸= X¾0Ê?ـ6Y½wÑ?¸= X¾0Ê?Å4ÙbunN?§"Ðk‡?ê²É§b¤m?§"Ðk‡4FGL J2323.4+5849?Ë>ªŽÃ€ÀéÛÑLŽÀ7'BÁE°
À:úïY­@ۅä°ï!?ýîy	×W?šKc™å?²³	¾U÷¿@5¿jäz?ø:Șµ˜ÿ?êVð§h[?ІÁOÁs¿Ø€Jþ€ùæ¿ÞýD
öä¿ãÒRþT¯/¿Û‰°b³ÔXOTHERsnr3FGL J2323.4+5849Cas A?çý';Å?Ä/x@¶Þ)?б‰úuÇ?Ä/x@¶Þ)?—ŒGÜ‹?«~ç1u/´?ïCÁÛ¨?«~ç1u/´?éåÉ	›ø?¯1£''!Ü?Èh۷ِ#?¯1£''!Ü?~äLDq{¢?m­"-J/?ïÂ7gw	?m­"-J/4FGL J2326.5+6122?ï£	Eå®!?Ì9Ê&)_À:â¢÷ç-À;Q·ê½xœ@›, šTU@3«ÉGO?Ɍ'sZj°?¤~=šZ?à91yõd?ÿÄ¡ÿ?í¾áÝU03¿áÚñR¾¿ê7A_ƺ¿ßÍbßHOz¿êÅV¶Jª¿Ù±Þ´Ö·OTHERsppSNR G113.0+00.2?î(åG(™Ã?¯Vp]è|Ý?­q«vcË?¯Vp]è|Þ?í±~/xæ?Æë
!Áˆ?²t‡Ü8Í?Æë
!Áˆ?ì4®¿û?¨n*JN¶·?¿NZŠ'`?¨n*JN¶¶?í²æ¹ªí3?œQZQľ?²hÊ2¨–a?œQZQľ4FGL J2333.1-5527¿ëAÿë‹ÀM)f@¦¹=À:I-(W7À<Žï¼»Ý'@í¬АÒ?ý»í·(Ú?Âz‹÷Åsè?Ô°"‡áá1@ÄÖÓõ¶?ø9‹¼â¿ÒÜ"'Z¿É§<µ¿Ü\2/ýô¿ãv=öÔ¿ë‡'aBæ¿ïý|Í°ø[OTHERbin3FGL J2333.0-55251FGL J2333.0-5535?¨Eã? ¹?©pIGˆý?î{¡ÎÌ
õ?©pIGˆý?Ô$ê4GVÑ?Ô¨yÐ×:?åíŠåÜT˜?Ô¨yÐ×:?§zÄ°ô??šyi0bJv?îˆS´ÿ€¼?šyi0bJu?ÐñjŔÀX?µa·¡I˜è?ç‡J5ŸÔ?µa·¡I˜è4FGL J2357.8+6231¿ëÄ;…Üh?Ó8ªŠÀ9IëoOCÀ;0Úb·…=@qC~Yø@èÞæªÄd?Â1›X‹‡?ƾ	e"i1@QBè²Ü?÷a,Ór®H?ïÐøuÈ9¿ât1€*²±¿éÚ]C§õ}¿ç…öº «¿ïÿ4=ŸGÙ¿ïåﳁ¢OTHERsppSNR G116.9+00.2?çl8(`Û?Ë@I³7÷?Ñ'Տ¯>J?Ë@I³7÷?ÕÆ:é'Z×?Õ{^r?bæ?åâ‹lR"?Õ{^r?bæ?áôgI7?»ü˜"lt?Ü1Åm'Ý?»ü˜"lt?¬ƒ3 :5Ø?"¹Š"̃?î7ÌÅü\¢?"¹Š"̃4FGL J0000.3-7355?ïåG{ÉÀE]a€M˜9À;%¦Ñ€ìÀ<ʞœ7ً@ÇÍz3£@f»üÊ?Çõ€ #v}¿®0C(É£?Û
ma'Pþ@ #¾ööA¿ïîa«ì?ìª'á›eø¿ãJ<߯R"¿àÖöâv¿ãڏÎ>¼Ô¿ïûSÞNjUNASNone?ïúÇ][ô?K¼žËrj£?D≊1;?K¼žËrj£?ïüüêù?H?TÜ)d2Š?8¨6ÁL?TÜ)d2?ï¦h71?†…Å*?†{eò3¹m?†…Å*?ïòÎ3#1S?N¸Ä´6?Zc™¹Yò?N¸Ä´&4FGL J0000.5+0743?ېÇÞ|F¾ÀJƒÅ?9ѳÀ:πhp+âÀ<t3⅛¶@»?ö;\?ýl½³TUÃ?Ø·G?Ëç?Þå¥vF®:@JFsBî@ÿ_Y¬Å?ï¦'ÊÖ(¿­O·½	úï¿à)HÎ¥êá¿æ™¸:lã¿ïÿãzŽ;˜?Ù­ µTUNASNone?ïôè]®Î×?aʱr=Ž?V/D¢bR	?aʱr=Ž?ïð³x5&?v?vE6*D?^™•³õC?v?vE6*E?í§°J·ih? ‡¶Ý×<?²Â}ªD´½? ‡¶Ý×=?9>\?w§‰ñZ)?‡q°z©?w§‰ñZ)4FGL J0003.3+2511¿êÞ¨GúyÀB4«ùiäÀ:¸üþÿÞÀ<|ÆÖƬ@šº²˜îú@v€$}Ê?Ð>.ϏÐ?Ԕ6ê'@\¯-•?ïÓێ¨ò?ïƹT繿à£h_Ýƒ¿à¿½‹ç)¿çk½¾<¿ïö({ILz¿ïÉÏ÷úxUNASNone?ï:ÿ'#?¢_Ì«T;:?˜ 
ۜì`?¢_Ì«T;:?çÀé
Ú7‡?ԗé¤ç'?Ð~-êKò?ԗé¤ç'?ê"ÅŠD—ý?«{¨Î[ ?ŬéÖí ?«{¨Î[!?Íÿ'©?°xZØGš?躼•¾?°xZØGš4FGL J0003.6+3059¿ßêeÞF¯À>Å¡fµNÀ:ô™aeu¦À<ê)\ðœ@fçŒí?ýK˕•(?Ìu9èÙó§?èŸüàõ–@é™Á݅'?ý})vpö¿ê!—à¿ßAJ¸Šöi¿¨€Ua¬{¿èïÎY"ǿ隢ãÅ6Ö¿ðUNASNone3FGL J0003.4+3100?ÔU­X±€?ɃbÂzt?åÕ)S§?ø?ɃbÂzt?̛€.}?Ð/ë0ëÈ}?èÙ_ô ?Ð/ë0ëÈ}?Ç8»}sÖ?°ñ'ÁNñ?ê1Ñ9 £
?°ñ'ÁNñ?ÇÌõºÉLX?±2z¬8؊?ê'M¬é?±2z¬8؊4FGL J0004.0+5715¿î°O×·ªÀj<´¼5À:
ö¯õ%±À;øãȑԩ@²á±
y@éÜÂä¿?Ée¶h1m?˽®·8@œC²Ý7~@Äó  ¿»ž#þ8?ï3À¶‰?¿æm4§§y¿â½˜çÂòX¿êÄò]€
׿ïý."hqUNASNone3FGL J0003.5+5721?à«HY†0?Éu{;þM?Þ©oÉLó ?Éu{;þM?í;þæ·`?ÄXmd‹1?¶ ØÊE?ÄXmd‹1?ãi=È¥E!?ºþ›G'—?Ù-"nµu¼?ºþ›G'—?鹙%õ­;?°#õÔ&‹Ò?É›h)K?°#õÔ&‹Ò4FGL J0004.4-4001¿åU:$]úÃÀRvñ€
À:¤ˀœsÀ<¤@è'œ&@M®$ëò­@Ò=ÕM¤Ï?Á(òg'Ñ?´Q
u#î?ñ
	n=Ë@\nóӡӿ؍«dGRO¿â
M++ýµ¿ßdb–£¿ÞÇCuö|¿éw±b
;R¿¨ˆ¤B®ÀUNASNone?ïü•mr?4g¢%&ƒw?;T—o1Š?4g¢%&ƒv?ïþuó™z)?Eë,&ց¶?( Æh]oò?Eë,&ց¿?ïܦ3NÔ?xŸÌ£Ö*Œ?q¬æX•õ§?xŸÌ£Ö*‹?ïþrT€ÚG?Ò>cƹ?(Ú·ò["7?Ò>cÆ4FGL J0005.6+6746c?æí>¹+Tù@ åæyF=À9»g
USÀ;8Ś©d@«sP¯šã@Üï$©Á?ÎÿöZdÐd?Ï}Æ_@ð?Û¸"@ó…PalW¿ãŸ£i&4G?îÏ`%Æ¿ç
.Ýc¿èéRáP¿ëžÙßÚƋ¿ïÿ/?ޒGUNASNone8?ٗߌÚI7?Ë5ý®@Ç?ã49'Ûd?Ë5ý®@Ç?Þ¾Få¡{Õ?ҝr9J5?à Ü/B?ҝr9J5?ש*ªà¿®?ºíl®"0à?ä+jª )?ºíl®"0à?ÞXÜÅåû?»hðJ""?àӑ
9?»hðJ""4FGL J0006.6+4618¿ÏñVf›!ŽÀ/½KÏknÀ;;·"¤%À<"g©\…<@ u™Y,í?ù,?£ƒþ?ÝQcŸâˆ÷?âi9Ÿ³äô@$ë7ò@?ù\ͶW¿ˆf_Ÿ;³Ï¿ïùš@¬ó?ímÿ"Z¿ÑÈýú1¿â%¢@Ýî¿ïÿñhUNASNone3FGL J0006.6+4618?ïÌÀ¾–Âæ?w6'1r$©?yŸ ´žŒÇ?w6'1r$ª?ï÷Œ£æ¬?p"XùèÛ?Pæ¹Ò2§ø?p"XùèÜ?ï^h…"ø‰?K(T$ôR?"2ï[ îç?K(T$ôQ?ïTx*ˆ?‡H¿É{ŸÁ?•pú¼üO?‡H¿É{ŸÀ4FGL J0008.4+6926?ï#¿ÝŠE´@Šü‹y£À:S\лnÖÀ;¾=‰ÎJ{@ Á<JÞö@ïþøþ"?Ê	¢Ö"0§?¸—=í§?ñi!—)|Ñ@¤5ÂÆ¿íÓbÙð!?ïþÚ0bž[¿å@£(Ž"ƒ¿åôûTŸ"…¿ÚW3£E"à¿ïÍbUNASNone?ﶃCî0Í?‰8l§­oî?'_/sÌá?‰8l§­oï?åµ!?¦'¿2yCí?‰'·¾©?¦'¿2yCî?îrq?'+?¡7K,AÚm?®¸ØìÝV?¡7K,AÚn?îþN•û??v!£q¹P? §àL?v!£q¹P4FGL J0008.9+2509¿â^…›ã¹ÀB\¿]xÀ:§e
EÔ À<K>I窟@îÒ09@" 5•
?ÏÎç"3*û?Èntý­ë5?ôÔb³S@â±³kÒ·?ïBO/èû׿Þf7l}ל¿êDP\8åû¿í}‡Ÿœ¿ïþž5àŒ¿ï€ú)&jUNASNone?ïö94긜?‹ù+é/í?S–*ŽÈÛ?‹ù+é/í?ï®Râ]ö?šG3%"Pè?"}ëGh'}?šG3%"Pè?î'QPÿ;?˜ðƒ¥*
¿?¦êêðE?˜ðƒ¥*
¿?ï7Ól"¡x?…­LîHP{?™'mkÑ?…­LîHP{4FGL J0009.1-5012?ßýÓÍüØÌÀPbç-¡"ûÀ:kõ²Ÿ$À<'ò®2®@ K¤ï
?@éÇ´_?ºÃˆ€l¡ê¿¿:_nÇÖ?҂ú;h@	S6Þ¹^?ïÿlýY\"¿×ö%ö4¿è>O ¿äöTðóÿêY*ÿ1£¿ïÿ"¯ý‰-UNASNone?ïýÈ d›?3>nό±?1¾üÛ'Q?3>nό¶?ïþ)ÑÑ?GùBû"ž#?-orâîõ;?GùBû"ž?ï›Ð6L‡?†1‡¬L-g?‰òlþÞ??†1‡¬L-g?ïûYzË=?3"E ҃W?B›òÓ
ä?3"E ҃c4FGL J0009.2+6847?îÕðÐÖH9@ðù£v'À9»œ`ô6žÀ;f?Èc@ïÓ^y@Zh+b"?É$•vjN?àÕJœ@iž»'?þ,­.vá¿Ý.Íb¿ß%"?]ä¿æ¬\꼡ܿì¥×€D¿ïÿ'`4P¿ïöU\Rç.UNASNone3FGL J0008.5+6853?¿>gÅod?¿Ùq
f@y?ì3R}?¿Ùq
f@y?¤nH®¦?¶yùZÜ×}?î¿	u˜?¶yùZÜ×~?IJ‰¬U¼?®"Âñíx¡?êÓ"ê'?®"Âñíx ?[áx}–…?jוÅ'${?ﺐz	¦?jוÅ'$z4FGL J0009.2+1745¿à#ÞíØÀEû‰a=1ºÀ:ÊZõ1À<ulC9@õ'ßÃ@fàÄÑUÉ?Ӊ7³Ët?Öüàü.º(@±FC±/¸@uQÄ?æPËßçܞ¿æ~ُRá€PB¿×¿ëb¤À>I¿ïý¯ùWoS¿ì0>·çUNASNone?ï´§RÞ¢?†"žÔý?'Ö:+HW?†"žÔý?ï®ß"Ã?•'ìäß?"H 8Ïe?•'ìäß?íÁ³
?¤ÉtOùK¬?·ñòg—÷X?¤ÉtOùK¬?îXN›i²^?"HXbJê¡?ª{IdÚ?"HXbJê¡4FGL J0009.7-1418¿Ü
ò
þäÀRz^³¾#À:y?Æ¿l'À<Žè´‰ßè@"êžnëp@{èäZˆ?¾ñ[¢h?¾}¹"6?ù[åô»ÿ@1är…Ùs?ïþð çkµ¿Õ÷Å^nuT¿éç`+¹Â.¿énlŒñ¿ÖÄ¿ðUNASNone3FGL J0010.5-1425?ï÷€2·ÈÃ?YÄ~¤s?PÿšnyR?YÄ~¤s
?ïô;¶$š;?qÁcuph?Wˆ"¶Ë‰v?qÁcuph?ï'¡Œö}ª?'æ¬`©Å?›Îa0J ?'æ¬`©Ä?ïÏÚ
7?i;/æ-†´?xúú8d"?i;/æ-†®4FGL J0010.2-2431¿æl½ðÃÀTô±î$5À;}íÎ¥!À<àINþjÕ@CÇDø'ˆ?þf ³iNx?×kWÅ®K?Å2äƒÍªm?텯¢šÜ@€­ê´iT?ïÌGkÏ[ó¿ç`.ßœ/¿åÎ=_Üßj¿¿ô/7w)¿è
˜à66¿ïÿ'¢."'UNASNone?ïýöN9âÕ?3%$Ù@­Ž?0MŽ0éY¸?3%$Ù@­Œ?ïû	ÔL.X?[Ç ýA©?CØ®ÏFž5?[Ç ýA©?ï°i̾ç?'-õ·7Öî?ƒåÐF)?'-õ·7Öì?ïñÕ+
±‹?P{J³»6?\U©äœêB?P{J³»64FGL J0017.1-4605?ïô$}ãÀQw_™Ã‹À:×íø–3À<©å
5r©@¼‰:Ѹ@*╶¶?Ã&LšãEµ?")ÛÔÁR?νÚÁ'ï?þ¿VGµK?ïäE#öN¿ê˜Ô½‡	Ÿ¿è–­Í-E¿ç]W>UP?¿ïþ‹ Z›¿çºñ£EêÆUNASNone?ïüñàh"V?F¸në§p?8pü»]Jý?F¸në§y?ï'߁:†?¢
èsô¸á?H>ß±^h?¢
èsô¸á?¢}hF?"±ìpYÓ}?‹`¥î¦?"±ìpYÓ|?ïd3³$?}ùkƐӫ?Œ&ó6û;?}ùkƐӨ4FGL J0022.0-5921¿ÚAꋷÙÀL°Èÿ¸²dÀ:sÕzñ7æÀ<XCëè@Ðu¡æv@…qŽ¸•?ÀŽzV³@	? !ÆyK›?áuÒ"4Ö@Wj^B«v?ïý)‹ê"n¿éb"¿H¿åVŒ¿ª¿åF^ˆ¦¿åDmþ5O˜¿ïýÒÞߞâUNASNone?ïýK6µ=?9K¦¢LW«?5¦JVöV?9K¦¢LWÊ?ïüâ9?üÁ?QtO¾7Æ~?8î6ÿÌ?QtO¾7Æy?ïë©*"†?eêúl?dVÕky~%?eêúe?ïé"#p/?S¾¾F\›?flÜíÐ}?S¾¾F\—4FGL J0023.6-4209?ÄÐÈq<$ÏÀR{½øôsÀ;kÿñÀ<ޟ›;ZI@â#P<@Ž­\Äüõ?ŕá"!¿ž¾¤k?Ú*Ÿü4C@ü‡ìóß?ìÁ?ûÅ¿êsÕº²¿ÌüòCÿ´+¿ã±L]üŠ€¿ïÿ Âg%?ïý<Á§TÃUNASNone?ïþnj•4ã?(>6€«B?)V¬±»j?(>6€«y?ïýŽ1‡sS?Q´KÙ'}´?3ŽsÄei9?Q´KÙ'}²?*¿·q?Œ'`šÃÕ8?\5P#Ò?Œ'`šÃÕ6?ïý§üN_D?*K×¾ÕÕ?2Àß?*K×¾Õ 4FGL J0024.1+2402¿ÓOÍÓ¦ÀC4äd™ÍÀ:ÅÔɐ¥À<œ!ªt³0@Þ|§E~º@$™Ì¢Û?ÁN«^½û¿q)%ñ£"?°Ù•³%"@V½ÝñL¿ëKYš¦	?çÐP~¿ê¯ ê[S¿Á"Š‹ßœ³¿ßJâ«¿ðUNASNone?ïþŠ}_g?,öo"f?'X*	Žø?,öo"f?ïþWV6È]?Mõ¾©"¶ú?*Šœ"z1õ?Mõ¾©"¶î?ïÚìpîº?wœšT²½?r‰ÀGˆ¢É?wœšT²¹?ïýbt-?(ÜͯW?4ï/Ô^'ö?(Üͯ=4FGL J0025.4-4838?ï%Ù¾dpÀPú¹©çÀ:ê"ŒòÂÀ<²ÄÍúÊ6@µ·O,´?ý$ÞÚ5?Ï/®™[_?Ñ0ñd†½I?ýèú}	@@eò†ðŸ¿ã%)Ô½\¿ç濇iì-¿Ñ"…=l3¿æÒSŸd^Ï¿á&á¶hÝ9¿ïÿ«çy÷=UNASNone?ïü0†¨M?>•½~àª?<{ʽ"¶?>•½~à¥?ïüØÂoÉ?Rñt"¨V?9?á쁽g?Rñt"¨V?ï]XÂn—È?ß±	ø*þ?"Tç²-ö?ß±	ø*ü?ïê†HÑä?W¾F`ݑˆ?ey·.ð??W¾F`ݑ"4FGL J0025.5-5936?Ü\«ªUAòÀL›â.]á]À:úŒð=ëÀ<bēBg"@äù~@±aCç¶]?ʾ=ö°¡?¯Ò_]ނ'?ãÁ¶¹eü@G¦(s<¿èºGúj"ɿᛃ´UÿåØ?\6a¼¿è¬x™nÑo¿ã(¥ߙX¿ç}YÇòryUNASNone?ïþ^ë‹{?'™7œ?*GO¸WÃ?'™7‰?ïüµ‰G99?U¬LL/ý?:SµÆ6,G?U¬LL/ü?ïà;è>;G?rÿ╙S^?oÄÁĹr?rÿ╙S^?ïø£Ž1É??õ ¿¦ ?MqÇ£8ߔ??õ ¿¦Š4FGL J0026.1-0732¿Ý§5t­É–ÀQa 1ί%À;%sW±À< "€,á
@ fÏlå0œ?ý†»¦3ÛÐ?ÎS!¥—(Ñ?¶ cbPJ?ì7p¿°¯‹@rãºzå?íOKÝyn?Ÿj¿çdq>[°U¿¶Šùm¿¡¿ìô$)ªô5?â2ªw7oUNASNone?ïø¿'¸‡?LÞF¢+ã?Oµõã?LÞF¢+â?ïïïtS¬B?z†¨ÔHPj?`‹¬S¿?z†¨ÔHPi?ï±Þ‹æ§^?'똣z}?ƒˆ]V(t?'똣z}?ïÉï8^íå?q
9?{cЉå?q
:4FGL J0030.6+0539?íýò•¯æYÀLiˁs2'À:5ÆTǏÀ;å¶BFÌm@&›–Ÿ@ßR@>´q?Àª"¾"y¿¨jԊ0p
?â¶Õ^ìŸ{@÷ç,Êc?ÍïRˆ¸ö¬¿è"NÖý¨7¿ìç,­'¿éÜp
¯,¿Àò§è;é¿ï÷íA·ZuUNASNone?ïø)Z™_?UšE¦·¤ˆ?OZ•šƒÞl?UšE¦·¤‡?ïíTnqmº?|~(Öµâ?b«'Ž'E"?|~(Öµå?îÞY{="?•p¯Ïa%T?¢hL'¿O?•p¯Ïa%T?ï÷bòÙ×?GŒúAFç3?Q:òLQ/?GŒúAFç.4FGL J0030.9-3618?îu…íª6MÀSõ¢œwškÀ;¹6‰)	À<꒽ÝEÁ@ ÷"	â­?ýºžavÙ?Ñ RÛÅ
;?™Émœ»	?͖z·]@΀×?ï_;#í?æë"²È?à
.A0÷Å¿â§Qa¿Ý1ð¥¿É°"‡äUNASNone?ïþ
­?7|?-'Mø­?/U,ˆBL?-'Mø­	?ïùŠ1ݺ?gÚ@4«Ò#?I×8‰ùV?gÚ@4«Ò$?ïâËvEÚ?qEÖe¯¡?m4‰ºç&'?qEÖe¯™?ïíâc:YW?X¯µ
 d~?bœÅ¦¨¢?X¯µ
 d4FGL J0031.0-2327?ÖÿiÜÖgÑÀUÃa@OÀ;ž7Åi+À=0ºö
³¸@]]àÛÍq?ùºÿèƒ?ÙÁ½|LØ?èžLa…V@
ù®º"e?þF a3÷¿ïÿãDÞVb?ïþ'AcL«?ƒ,ì6
qò¿âmSà§Ë¿í&ÕVß	æ¿ê«ßí;^UNASNone3FGL J0031.2-2320?뗝D*s?¾©G	­– ?Á£ŠïV1?¾©G	­– ?íɝ
ÀÏ?ÂJwŒí›q?±·ó©ùŒ?ÂJwŒí›q?çÉô' 
Ð?³ørBßÎ?Ðl°¿ê`?³ørBßÎ?éà̆wÔå?µ"âUæ?È|Íæ ¬h?µ"âUæ4FGL J0031.5-5648?ëø7
MyÀN/Y‰ßÀ;0zW´ò»À<Ëo¤Ó‰@ A2û*?þˆåo®?ÌYO<(OT?¼\iãH;?ò@€"С@k–$ÅZ¿íYqýÌI¿Ùc"úÎg׿ۑÙüᨿà}ßÊÖS¿ÔNád‰l¿ïûs¾¾—*UNASNone?ïÿjZ'à-?†Io±É?´­Ãúo#?†Io±Èž?ïþBô…b%?KegþMÖ?+з©Ý§F?KegþMÍ?ï滪¸zÌ?q­f	ù–Š?iDUG…42?q­f	ù–Œ?ïü.ä'Á?1¬WˆÂ²á?>ˆÛi÷Bß?1¬WˆÂ²Ê4FGL J0032.3-5539?é–C	-IÐÀN á`؇ìÀ<åÏxÀ<ñ#¬­r"@$ïW'.B3?õhB>hñ[?×ñ¿Ë\ŠE?º	Þ%9Ë?ÛB¾@—õ«@#°Ó@¿êð8ÂiF–¿ïˆ!!7Þ?ëjé]Q>â¿ÄGûa@b¿ïéØÖ+?ïâ±pOô4UNASNone?ïÿ¦a
ȁ?
'žïú4?g½Ql?
'žïûË?ïýj
è¤?R¯åÊ6l_?4¯"ðºçM?R¯åÊ6l`?穀87h?†ñØãª3?…šñò%þ|?†ñØãª.?ïú³´?\AބÀ%?Gÿµ3‰0?\AބÀ 4FGL J0034.6+6438¿ÇNÄ(?ý7ú'ص8À9›[ÖÀk•À;hb{[@<©ÏÜ@ø{,Ç?Ã؞<@£?ÄW'afÍ?@yà{Ö:4@‡å‹_š?ïöòl¬Ò¿ÍkàÊÆ¿æٚpY.o¿æ
ë­òí¿å[LVñ¿ïÿöµšUNASNone?ê"Y"òñ?À+Rg¨†â?Ų›±°4=?À+Rg¨†â?àÓG-S?Óæqeê'ð?ÞYqù¥YÁ?Óæqeê'ð?é/ª…·lÍ?¶¼¡ò‡Å?ËAUé"LÐ?¶¼¡ò‡Å?æ¾á'k¥·?®gncÛ¢¯?҂<û(´'?®gncÛ¢¯4FGL J0035.2-1739?ïôrp ttÀSôÏþ°t§À;–…AÂÀ<Ù¥o±"@!\Ç
Àù/?úËg<O;§?ÒßÝ5¥©?´>ïÔäžP?äYaϨÊ?ïœ,@¥·Š?ï÷òµ"¡ã¿ë¯8gOšr¿ÛöÀ›æûÍ¿Çÿfèle"¿à­ëá$
¿ÑGã¤)ÀnUNASNone?ïÿÚæLH>ø$gUÅ+>òúÙÜ3°>ø$gUÄ«?ï§)H®#?™ ^[û¤?†95­Ôwm?™ ^[û¥?ïèºó9?qƒàxLq?gEáçÅÊ?qƒàxLp?ïŒÑ	<ÿ?Û,¡ ?ŒË½°ÿ??Û,¡ 4FGL J0037.2-2653?Ўl°Ô¿ÀUµI''>À;¡éhäÅèÀ<¨,¤£¸×@"ðE¢Ìs?ì>vþdŽ?äy(_ð€†?ïäkß÷÷É?ù–wƒÅ?ýû†5ä"h?ïó°0´Ó²¿äÍp@"Õg¿ß{W#ÓCß¿ØÇáÖt@¿ïÿÆTǏ¿Í¥˜¯cÛUNASNone?ïð?eh•™ci?`øaðX?eh•™cm?ïÃî= '?œáIÐà?~áxïìZ?œáIÐà?îa"õ?šò;3ëV?©ç¶ ¯¬?šò;3ëW?ï®Lô2Gø?ƒÉ6æ<?"lÂóný?ƒÉ6æ<4FGL J0039.1+6257¿á¤¼¹9Å?¿4GÛ5ñ)À9Xº'Gm}À;ß|ÊUú@oeÉÞZê?þ|óÁ-\Z?¾Í³ýsß?áú|2€…Ì@ Üa•FN@åÄè4Ý¿áP"G!ý¿Ú祖'R¿ÈëJw—¿äÉ"=—*¿ï6©Àd¿í ˆ JxIUNASNone3FGL J0039.3+6256?U#Ílôh?^¯;^Ìæ?ïõnI±?^¯;^Ìç?yô\3­Kþ?Šœ)ôïZ'?ïÌG˜¥h?Šœ)ôïZ'?ˆ?ËX;'ç?p°î•Ñ60?ïŸҟ`?p°î•Ñ6<?fBŒÁ?S#õ…ÛM$?ïéê½s>ç?S#õ…ÛM$4FGL J0039.7+4203?ÕÒ!'{À4Áæ>ŽÀ;4ebZhÀ<yÏÛu<@È8ªky@ãp¥"‰g?Æ~ÈÈ[N?—Œ|ù?Ò¤_۲÷@)N^³¿Ûè®àR»¿ÊCBtï–%¿êbÙð!¿áîmØJ¯¿à?ûÞ]Bü¿ðUNASNone?ïùyËÙÄ?IîϚ7ö?Jӄ˜ñm?IîϚ7û?ïþfŒŠÃQ?LE¯v™t?)—7SÊí­?LE¯v™?ïµÈý«…X?É·t
é?'À•©Æ?É·t
é?ï÷ÚÎЦ?>²êò?PJcþ^µ<?>²êòy4FGL J0040.2-2725?FÀÞÉÀUßµà÷üüÀ;BH­î»4À<|ڀ·@jõ['@‡wÞ]îÉ?Å^j™{炿ª Xz•rn?ãö«ù®r?ùÜÚ
Òüg?ïÿýaw¿êÖa +n™¿æƲ×XA
¿Ú~YÝA¿ïÿã_¶Hý¿µ	-%RUNASNone?ïýcvg~š?<0±_°?4äLÄ0‹?<0±_Ë?ïJâ‹Ü©—?©h*œ3?–£®"jÍ#?©h*œ3?T¬?…cgã0D?ˆ'9|êÔü?…cgã0B?ï"-Ÿ.é?R
5iƒë?‹4˜4y©?R
5iƒí4FGL J0040.7-7157¿éÐsŽ¼0ÀF'³¿µÀ:ëHɝmÀ<±'¥‰'å@ ¥×Û?ý%=§*|?Ì&ÝåMø?ÕI7º@fÚå"Cï?ùš¥]G.?ä)€,
¿ïA["Ì´?é±Ç2ŠA¿áPÍ ¿æh›ÊÌA¿äÀ;#Â|èUNASNone?ïÏ4±<Ÿ!?z'±4®;Ñ?xe§a°oB?z'±4®;Ò?îíÞ!{??·Þ­…úÀ?¡"èNü?·Þ­…úÁ?î¡6©?™¡xa©Ý`?¥î̕næþ?™¡xa©Ýa?ë.ÉVø›?±0Ÿnat0?ÃDÚ¤"¾?±0Ÿnat04FGL J0045.8-1324¿àÉ+n6þÀS
¥¹bŒ½À;§/F>¨²À<ò×;»—ñ@ rj Z=Ž?è×ÄýËrZ?ñ')bÏÙ?ì/"YÒÚ?úÀ?ö@Wÿ÷òjk¿î'ËâA(>?ïþCÒ½§–¿ìCʟöÕà?Æ#ˆIe$¿æÅ&p­¿ïþz#²Œ°UNASNone?ïÜÞ(1Ÿ‹?qžSÄ~P5?qëç0;?qžSÄ~P5?ïù~Ӕ££?m¨˜ÖóV?J±­qs
?m¨˜ÖóS?ï;£ûzf?'Å°"%¬î?˜‹€½ÓJ?'Å°"%¬î?ïîòç
[?c¹#ˆ.­?ap
ò¤¨?c¹#ˆ.­4FGL J0045.9-2021?áÔ?c4
ÀTÇƧÀ;2/Ú¹šÀ<Ƨ?tŠ@ 5jE8?þõÄ}î?Èüí¦â'?¦GáýÛ9?áíÜçÍS@‡
íC峿îåNCZ?ïô¬ç#¿ânZ†^Sr¿àL0Z:ß¿Ô&2™°?οêT^/
ZUNASNone?ïý]gˆ1?0!'þ"ú4?5ôþm{?0!'þ"ú-?ïûö»?Û?^ Ô°©ÛŽ?@%»"?^ Ô°©Û'?ïå¥ï¹ü?nmz5|ˆï?jZFð1?nmz5|ˆí?ïøU Ñg?CKmLàX?N«}¼ºc_?CKmLà[4FGL J0046.7-7048¿Ô®×—¾#¶ÀG'ž@ÈG,À;œ¥R4€À<ÒÆ»:Ô@Ӑš—@¸j$aY?ÇÖÎûtU¿¨ÍÆᕦ?â³þÕ]•@¢Äþ¢1ï¿ïü]Ä?ït£`Aß¿çÄyA¿àèõW/'¾¿ïþ5Å´ª—?ïöÇ<jšUNASNone?ï󭑅ß?Xëè§+3?X¤Üôà@¶?Xëè§+3?ïå4œß3?ƒmY¸p¹?jåËc Ìü?ƒmY¸p¹?ï<bMR?‰}ÉÌë?s¶U½ß?‰}ÉÌë?ïÚ¦´ëH?jÈóÍùF8?r¬þ¥Š\?jÈóÍùF84FGL J0048.6-6347¿Ñ¤L_ÁfÀJªÄÑ¢À:ÇK^£#†À<Çdl'"Ó@)?ý<Aÿ~Ñ?ÇÎÔcïé‡?ÚèŸ%ʔä@¦Kaþ"@.ï\ڗ¿ð?ïÿÿ)@k*¿ÙHÅ×Eî¿ä¿Ä}îB¿èÙXáÃ~ð¿ïû²]µ½½UNASNone3FGL J0048.1-6343?Ù®1\ô:?ÈóìÂ?ã(ç?Q…á?ÈóìÂ?àDo
¶þ?Ö¥K ?ßw!ëö'?Ö¥K ?Ó‰¢á8b?³ŽceR1¥?æ».cÏ?³ŽceR1¥?á[šQK‰F?ºéjÙ¿¬?ÝHË]híu?ºéjÙ¿¬4FGL J0052.1+6444¿ìB´hïÇ[?ýíözE@À9y\–$À;Xfêð¤B@•ËÊï'@è‰͟[?ƪH(äj?Ñ-P›#•@Ý ×ç?öؤ^™"d¿Ô=ՃT³¶?éµ{âÏm'¿ß§›š¥³-¿ên¶—b&¿ëRæ÷ñ=Å¿ïݥ̈́'±UNASNone3FGL J0051.6+6445?½ªôsR×Ú?¾¶J0"æ?ìJ¡q•¥?¾¶J0"æŽ?µKÈId
ü?ÂÞFˆÊ¨??íV†öÓ~ ?ÂÞFˆÊ¨??Ô96Ó«p?µ Žj»?åãd–*7È?µ Žj»?¼õuG;?¤»³1«?ìaQ]œ×?¤»³1«4FGL J0054.4-1503?浿.º>ÀSz îõÀ;íNäHÀ=]¹ïzw@!'|`Â8?ôÈ͙{f©?âf~x+
?êT•ƒŠcœ@
ŠBä?üù'ó¸¿ïÔwéR?ï}WÎÂ?ïéR‹¾?Ò¹,;È-+¿á‹Y/F>©¿ïøu'ST;UNASNone?ï([-d9Ú?›)x#ã͔?šôšSxÄ°?›)x#ã͔?ïSöºÅ?³8‡P:$È?•(­ç^j?³8‡P:$È?îHüsÃUÑ? Ë­ÅÚá?«p8ÃÊ¢é? Ë­ÅÚá?íNrRóE?ªÕ¤Â5?µŒmhe×í?ªÕ¤Â54FGL J0055.7+4507¿Ö—µqM]`À1½šA_EáÀ;ùÕm…>™À<ý3þ4Må@"¯e3?÷(ÄDhÝ?ß÷×\È­Ù?æS"ÛÈ@a.á"Úî@$m/ƒPW?ïÎT 鄓¿ïÿûÞ]Bü?ïÿ)vP¿ÍkØUÁþh¿Ì¼Õ~@"¿åÓ6þï´®UNASNone?ïå"üAY?jºJ¿ïm?jݾ¦ä?jºJ¿ïm?ïòúŸ1Iæ?{8ù¥0½?Z
Ál3o?{8ù¥0¼?ï`	Ò
Dw?Wœ'Õ U?"þž·q?Wœ'Õ U?ï3cQå¸I?'ìÎF"F?™"•ÃHöó?'ìÎF"E4FGL J0057.5+6814¿áð´<´äa@{ÔÝ<†™À:aGzÕÀ;'Ö*'ò@4¥Ó
ه@ºNz·VC?΃†d9»?¥n…ž?ßiÈñuù@¯>dÐÂ?Á+¡C‡Z¿å­VŸôÒz¿ëŸH˒:¿åTê"H)d¿ëŸ¤À¿"j?µ§\лnÖUNASNone?îßå€8Å?Ÿß×Ò°?¢§ü~cÅ?Ÿß×Ò°?ïg=õt‰?°yýÓl?"A^1nã?°yýÓl?ípF"¤ð?¢'öZõvŠ?´}ÎêØ ?¢'öZõv‰?ï—îE³±¬?vå"â•?Šn""ñ?vå"â•4FGL J0057.9+6326¿Ú¦PùN«?ânù´
3À:{›eK´3À<-yøêb	@"óXˆØ+P?õ~€Ǒ$?̾ywæž?ÌÂy6͜€?ùۑÁ^Á@pUÚ'(c¿æòI~N9Ÿ¿êÊE3÷Å¿æÅp'Iü¿ÔSÈ
L4¿×Á'è|U¼?´°bÞÇv!UNASNone?ïçºu-~/?o,NÕïj€?hEŠÒÐ}?o,NÕïj}?I¾òD?¬³>'w?ˆZ­Co.?¬³>'w?ï.µk%?•F¼-ŒÚ?š)R›OÎ)?•F¼-ŒÚ?ïå"oòA?dìí̜n¼?jl
¾€¤?dìí̜n½4FGL J0058.1+6915¿àþoUú$Ñ@–tŽGVÀ:AVZ¨WÀ;¶o×ÿ/ö@ÊæØf³é@˜±¨ó?Ê$²;üÛ]?Áiànj?ó0¥i±t'@¥Ðȯܧ?ï,pk¢æI¿æÌs 3&H¿åM÷¤ç«u¿évØa´P¿ïÿáåÔ?ïþø™q¥UNASNone?ï´¦CTø?Œ$4Tܚ?'Ö{/*ÁÒ?Œ$4Tܚ?íÜßc@R?ÂÿÛ Œ"(?³ñåýq?ÂÿÛ Œ")?í7j7ÕD?¤µœÞZí
?·vD®AUâ?¤µœÞZí	?í±=>€? ±Ø!è^?²vÿ׈? ±Ø!è^4FGL J0058.3-4603¿æ£"'XÀQÁqKœ¶…À;µÀ_@˜À=BûÅ@ô*û×&m?ÿZÊ¡yaì?Ú¢w{?© ÷œY<‡?ÊYƒ©î%@YÅM~¹?ïaì¹ÒE¿ëlÎàM]+¿Î	m&žû-¿ÜSa[ºà¿åG®záH¿¬U½KÐcUNASNone?ïÿ°m¨?ÿ;Kå»?ä»þV,N?ÿ;Käw?ïþq+ã^3?FNÚØÕõå?(íAÊÖ<?FNÚØÕõÞ?ïðÿf"¸M?s¤VdýRI?^3ºeþ?s¤VdýRE?ïþ¹êQÛÎ?½dI'´É?$aZâCE?½dI'´ø4FGL J0059.4-5654?äÐó¹4kÀN°ËæÀ9¹Â^´Á=À<êAQÚ@vr€ó@¢ÈY …F?³K¯ÁN>|?É·¾]HZ@Ú­Å@§Ó"ý0¿Ê]%Ÿ÷¬Ÿ¿á¬M P¿ænij&å¿ê–a¡Çæ¿ì6ÎÉ&O¿ïûÛxa:­UNASNone3FGL J0059.1-5701?î
õç3«Ý?°æKmÆf?¯ ¡ŒÅB/?°æKmÆf?îõíF«R-?º@øý)Iª? ¡+•JÝ3?º@øý)Iª?ê}mܯUª?±CfÌD'?Æ
HB©X?±CfÌD'?ïý"
 ?‡eW/Ú+?_í~¬?‡eW/Ú*4FGL J0102.0-6240?çk]R8EjÀK3¡fµÀ;eTÑél@À<à£ó¯5@ N:¶?ý»ed®?Ët˜Ù*S;?¸½ÔakªÉ?ðuøÅyu@*AeûÝ\?ìö—€º¦?ÔüÍÛëx´¿Ú}âïN¿ÚÁ1æ,¿æÕ)' ¿É :Š¿âUNASNone?ïþ½y•ý?h:V9¥1?$(f /ë[?h:V9¥P?ïýx¤?P·Çäþ$H?4?'ß,²?P·Çäþ$L?ïðDc?k*Hõ
2?_w9çñô?k*Hõ
F?ïðö›Oªô?Ny;%`=[?^É`ªã?Ny;%`=Z4FGL J0102.1+4458?ç¹+ÁñÀ1ܬ¯öÓ1À;@e+ÓÃÀ<®Ó5œš@ )çJ?í)•€r+?ݾ¬
9¤f?ëìjŒeÔp@<¥¢¼@¡¶É€<%¿ï£'Á¹m?áÎϦ›àœ¿éçzBfV÷¿§k®yÐ{ƒ¿âXxgꍿïús™TÐ<UNASNone3FGL J0102.1+4458?ï‹­&|T?€"ÈøÊã°?~º)lÁÖo?€"ÈøÊã¯?ïéÚZÿJ?˜lQ¢¾Ç?f%¥ð¶œ?˜lQ¢¾Ç?ï3òÙ=Šw?'v	¡,?™¤ØN±?'v	¡,?ï½hÿ0A1?xšAŠÄ˜?€¥À3ï³Û?xšAŠÄ˜4FGL J0102.3+1000¿ÄA1ïãÓÀJaä¼­šØÀ:µ¸•Þ#6À<aÁLf
@ œ¢»×1*?ùÙú—á2µ?Ò[ÈRèÛ?Ú³ô#Rë_@˜Cæߞ?ýqÆ^s¨Ä¿Û®ž#/—¿ïÄÜ"«%³?íûÀ«+g¿Ò†É]VF¿æ4½vît¿ä íìEzUNASNone?ïÐVÇf*V?w¼à~ûV?wԜLêÕ?w¼à~ûT?ïÈÇ&Õ?Ÿè_ÌÑÊ?{÷ul•²?Ÿè_ÌÑÊ?î²
\ÒÖP?='" ?¤ß*2Қõ?='"  ?î^m¬V? X†Ê®?¯º©%:£? X†Ê®4FGL J0104.6-0818?à$õýµ…ÀQ»<`ŸÀ;	7·&rÀ<ƒM#ŸA@/x›æ@¡Ñv€?Ö ¡`7x<?µ¶|~UÆ[?àˆÅ †l@½6	Í¿­g:f¿í»Ó`Þj¿Âe?	U>¿äÉùHUÚ'¿ïÿîͨ"ß?ïž^z^ÁUNASNone?ïö5I¼|–?XÀ0+íö§?S•l‡Ô£?XÀ0+íö¬?ïì¹ý;š?|¢•/§ßÆ?cFÄþg??|¢•/§ßÆ?ïN­Ó›?%ñõÜh?–*Ež,¹?%ñõÜg?ïôâ‹L¬?JýŸßs‹?V;Þéf¨;?JýŸßs'4FGL J0106.1+1131¿ïÐLXsîÀI–áïsÀÂÀ;ez¤£À<ºÓø:9@ [ž·:¿?ý$™ù;?Ò;9\B 6?ÐX9™…x?ùO¡(TH@ç`Õ®?ë<7Þé"é¿ïþôœõn­?ïóeRj0 ¿èä‡Ôu7»¿Æek"£'¿ðUNASNone?ïþ€L\9?*Q}ðý‡g?'û:?œ{Ù?*Q}ðý‡T?ïþÊÐm?Kya\cÊÉ?.ƒRþ©6É?Kya\cʺ?ïxë×J?Š¿ÜVЈ:?âœE¿P?Š¿ÜVЈ:?ïøžÙ}mu?GV{æë§?M"š
J.K?GV{æë¦4FGL J0112.0+3442¿ÞU¸€¯›bÀ;úÞ]	À;/6oþ•À<µS,;d@Q#RŸÊ?ÿ×_f˜?ÙüxŒØ"?Þáp}–ƒ»?üÞΌÀmC@
?ىʿî´¡'¢?クAûM¿ÞÙ§{¯xÔ¿ä ‹Ær?¸¿ïÿ«çy÷=?ïüK_ÏÉVUNASNone?ïÍ1*ù¶?'Ÿínå?ygj¹%?'Ÿínæ?ïÝxý—˜ð?Œ–eéZE"?qC43ˆ9?Œ–eéZE"?í[¨ô¯?¢ü§U^)?·Í"¸_¢‡?¢ü§U^)?ïP¶£F ?ˆuNOm²¨?•é+—>‹ó?ˆuNOm²ª4FGL J0115.4-2917¿á²bX°¯ÀUvÈ´9XÀ;‡ÚÙÖÀ<äÔÉ'@ µQù#?ûûI·Ùö?Ֆ¬Ÿ…ÁË?Âß#¼r·ƒ?ðZ%Ðt!@Û¨!Ç¥ñ¿ïÿC*!<?ïéÿºùf¿çÀèÞ%d¾¿·½WÓ{"¿ÔÝ[û©Y*¿èÏ^bùUNASNone?ïþ±'n?*û‹Ê›;6?.´çÙ	?*û‹Ê›;4?ïüŽÝ|F?[¦óR+J%?;‰-ÒË?[¦óR+J?ïÝ5$Õe0?t4
Ñ?qem•Mg'?t4
Ô?ïúsŒ¦4Ó?>éxæ;Å?F1Íg,²B?>éxæ;¶4FGL J0116.8+6914?ì{b]–¤@ì !sOÀ:Eûg¿,À;Ó2ӑâì@®Gp­@=Û	íÀ?Ò`¡üi?éÃãŸw),@Š˜í¢/j?ôå~I‡¿áWR'ú¿ÞHTbWãí¿éÜG^cb¦¿ïýÅÞFî¿ë~Ïu¿â©¬ ÚÁUNASNone3FGL J0116.8+6913?Ö	¤ø#?ÐUÑÆŠ?äû-ƒ÷nu?ÐUÑÆŠ?½lÿp–?ʑ'µ?ìR`í??ʑ'µ?Ú¬ýß!Z?¹vSI4?⩁oRÁ?¹vSI3?z
4$Õ~X?jrœž²?ïË嗶U?jrœž²4FGL J0118.3-6008?¥´ŠêiÏuÀLUA [ÀÀ;Ëô_¹À<Üò@úœ@¹±Y¤·@&Š"lXï?ʇSÆы#?Ǖb¨@ÑV?ü°Í'eŸ—@m-Dܨã¿ï"Eg]Ñ?ïÆlËÛ5E¿áÅ|vs#ä¿àހ("Y¿êͶ±Æa¿ïÿ¼®q—óUNASNone?ïûW¿<?CÅÈ°Ã7?B£Áþ?CÅÈ°Ã-?ïýŠW¤ƒ¬?RNja¼?3­BÛâœé?RNja½?ï+¯s¨Yƒ?'÷Ž€½f?šŠŠôώ?'÷Ž€½e?ïõ1¯u?J±ù=ÁL?Uœ¡Ì7?J±ù=ÁL&4FGL J0120.1+0505¿Þ»¤»2ÏÀL…£~õ©À;1bZh+cÀ<aG¾Ûr'@Uë²;|@ÿí¦a(9?Äõ¹NjÇ¿¸¼öëÚ.?òÑ8×·âZ@¨«B8‰´¿Á1³VY(¿íáqŸ¿á_ã*cǿ⼫™Ÿ¿çª£	"¾¿ïÿ¤DîUNASNone?ïú²¥U¥6?B7ê€Pxk?E5j©k&W?B7ê€Pxk?ï÷ O'®B?jN,3P·?Q¿a°£}Ç?jN,3Pµ?ïÆÍçÿ"\?|¥Ž–û¬œ?|™5Ñs?|¥Ž–û¬›?ïñ¨C½??MEJælj?\¯ïx…'N?MEJælp4FGL J0120.2-7944?îÚÑ4L«ËÀB¦>-b9À:ÛWvšÙÀ<-"¶³…Ô@L>7±@®åD'×?ÃЀ¶sÄô¿·gɽέ"?øʶ!œÁ@BÏÁ+?ïÖ%œq»¿ê>
A¢a¿¿äè%þÂ=R¿écÑÌk¿ÊÉ>!ù¤ò¿ã+ÕÁh¼UNASNone?ïþûS
‰?2H‹>?.`JÏ'w?2H‹@?ï÷ĒvO°?qcïsÊ3Ð?PvÛ`¡g?qcïsÊ3Ð?ïÃ¥e™Y?}©äÄíÊ,?~{­M3Sx?}©äÄíÊ)?ïõրȡ?J"FnÈô?TxÒþn¾s?J"FnÉ4FGL J0122.4+1034¿ï¤ªUMâ"ÀIÇ:Þ"_¦À;—KÔèëÀ<È[Q_n%@"5Ï`ûÃZ?÷{Ãà•®?ÔÔÈ#š¹Õ?Ôwã¼R?ÿC;¾òïv@aƒ~ûÉ¿ë-Óî'¿ïÿÿ>¹ú?ïÿç@ìYZ?Ô1ÄPÈÅ¿Ýbí`>¿ÖöçþV‡¡UNASNone?ïýEi×r+?2u?Ã
	?5Ô±Dn°?2u?Ã
?ïý½"röŠ?P©ƒÊìO­?2ÜhK®Q?P©ƒÊìO®?ïØË:6-?w(:?ô?sšqâäéš?w(:?ô?ïúg·]ÁÜ??cµÁiv~?Fa"ˆø??cµÁiv•4FGL J0125.3+6820?í|q,c@³çÑ5ZÀ9ÛîùûÀ;x¡L'H@¥§Yޙ@´hqH?ÓL.!%"?Ðü^ØP@¼½‹j@&¼<
L?ïÙº`ú?ÎGŸ{ÛË¿ê×2K¬¦½¿åÁ'¶ÿ.¿èЩôg¿ïüuÁù	AUNASNone?ܹŠº±1?Îî´S=ß#?á£t:¢§g?Îî´S=ß$?ÚÁç2Y1?Ò™3<£?âþŸfÓf?Ò™3<£?ށ´þuR?·ôò'‹Øä?à¿%€ÀEV?·ôò'‹Øä?Õöjòæ5?¶ìwø>ET?år"ʆŒå?¶ìwø>ES4FGL J0125.9-6303?àn\XٝÀJÐ\
V›À;D}¿H€À<Þ\)̂$@¡·â@ǧ¡š?Æ®^øˆèF?•ECV1?ѧa5úä@•èÞ%?샮uɱ¿â/-êôÖ¿è"·õ¥3+¿ÜCÄûÈõ¿å Ž¶È¥¿ÝVÁÃ.hsUNASNone?ïö<ŒY?JÄ䅋?S†çõMÍø?JÄ䅋?ïùý,@¶?a¾8¡š£?HNý‰(Ù?a¾8¡š¦?ïçÆà)¤?pF-Ÿßù?h9Öþ\*?pF-Ÿßñ?ïòmó0—?F´ÑLI?[$ߞÓF?F´ÑLC4FGL J0126.3-6746¿ëp\Aë'ZÀHJä)à¤À<D'À=-®Õߛ@!óhbêÛÖ?÷Æ5µ?ÚZâ9E›ì?҆êCM?÷ĞDú?û/,xƒõC¿ïþ…A¿êvjXŠÜ?ïûÚÂXÖ?À{ÝÆðú¿íƒ>Ò£¦?è	K¾DsÍUNASNone?ïø؄¶Ów?Q'CJ(­?Lí$²$:?Q'CJ(¬?ïøŒ¨ ÅD?jR—VûÏ?MÍ]|êó?jR—VûË?A(·7?—ϸ>t'ò?¤•ítŒ‰?—ϸ>t'ñ?ïß9!²°?kLXâz¡Ž?pcxï&§Ç?kLXâz¡Ž4FGL J0126.8+2412?Õp†cN AÀBú€If{_À:4ÿ—$tTÀ<EÔº.@£øÿ%@ƒCÿF?¼®î?Ž5b¿~áè÷¤<?³ðëºù'@êt¼•r¿ß^E"^ǿ䢅›µÓŒ¿èLÒJ»¿ì(S 8"¬¿Ò`P'yl~¿ïþÁÁÖυUNASNone?ïÿz¢…W¹?nñ+U?«¯U¿·?nñ+˜?ïþ¹§Ǟ?CuÓþ'w?$eƒ†E?CuÓþ'w!?ïèŠTk^?i´_0"r?gu«p"¡?i´_0"i?ïÿ{A"6X?ÆÏ[Yë?—Í™4ôo?ÆÏ[YëÅ4FGL J0128.1+7542?íEò®1ÐÄ@)ÿ]5e<›À;,$8Äl¬À<žÏœŠå¢@W­~'ù@cYÿOÖØ?؉$Vv"?îš#A΁ƒ@þÚH¶R@ݲ"L*{¿ï‹oÀbV?ïâù)L)¤¿Ü¤K8ãv\¿í8"†<Ń¿ïþ¯çÜô?íHúåäËÇUNASNone?æhê#X?о'¯z®s?ÓãÕ.+¹R?о'¯z®s?ׂ'¼Âß?Óø¬î4Pw?ä>¶ü¡ž?Óø¬î4Px?᷒.eÍ?¸4S‰‡$c?ܐÛË£4g?¸4S‰‡$d?ÐêF‡|ø­?¹Ý†ÜaJ´?çŠÜ¼Aƒª?¹Ý†ÜaJ´4FGL J0131.7-5346?àw½Eûg÷ÀO*êt}€^À:¿¾Ô¼…WÀ<µâ;ÉÚª@œ,Œ@6&˜ðý?Ñï ´«m×?ќã›EkD?ú:¹¤ÑÜ@×'n®ß¿ÕLýԺؿß]"Y¿ÜYãÜþ¿éâç¡'û¿é,Š'O{¿ 'ðpUNASNone3FGL J0132.1-5340?îÿàAª;i?¡2I$ü? ûå\Il?¡2I$ü?ïÜb	?'>˜åªA«?q÷pNû1"?'>˜åªA«?ì<}…%ÿ»?¥ór>ÏØ?¾ÖÐ?¥ór>ÏÙ?ÀÞúñ?}1	é§B?XÈAC¦?}1	é§D4FGL J0132.1-0956¿ïäêR‹ÀQ"KâCÀ:>_ïSàÀ<]o`
+Ó@¯Ûbç«Ë@'¤:Œ?²äôQ ?Ô.;&Ǖ@TbeOåñ@	šhÓ(0¡¿×Ŕ~ýŒ¿åŒqȚ8%¿ì†ƒý¦"¿éS>Ïu¿îáGB´°v¿ïóímVD°UNASNone?ïÚëågX
?xÄz£¸?rŠ
LSù!?xÄz£¶?ï°Úø"û²?¢–O¹•›,?ƒÉAÚÁ‰?¢–O¹•›,?íŸ*ŒO? -/¸ñe?±Ò>«ŸU†? -/¸ñe?ïmç÷£?ƒœì{þ¢º?']£Á¬?ƒœì{þ¢º4FGL J0133.0+5931¿ê'Oâ`ÀP!p"À:Æ(Oªb?À;Ó	¢z@ -Zk[mº@ëùŒHx?Âcwž™¿µ§â1¸ß°?õÄÒG`â?þ-°€0?îIDíoڃ¿êd%¿]"¿êŒ77…¨¿äãÉª¿ÝÖt{'H¿Ä™¢}îÃBUNASNone3FGL J0133.3+5930?ïÍÏõÔÉÆ?€Ày€"Dw?y›-?€Ày€"Dw?ïr9ñ5?¬om-‹^?'¿8Áߙd?¬om-‹^?î×Ýz5¯B?—zÄJ?¢'(\¥ù?—zÄK?îû¬çÐ*á?‰+¤¯c? E1'ýQï?‰+¤¯c4FGL J0137.3-3239?îUow'¯?ÀS§ÃÞ灄À;eEW"&À<Ízí(@']gå@àâ-‡"?ÑB	D¢Ff?ÈÕd.'Ü?ó^"ð•)@sÔ
ƒ¼Ž¿ï‰µ@>3—?ï1g`âC¿é<6a»Ü»¿Ì÷iCŸ/¿ð?ïÿÿ" 5•UNASNone?ïðáŽ?j÷SX[‹?_ÑñÖ<â¦?j÷SX[‹?ïØ-CHÈ?‹+¦	*ÿM?sésÞ[œ?‹+¦	*ÿM?ît¹"øÝ?˜üí3€ó?¨´g°2%?˜üí3€ó?ïäs?eA°}‡ÔÚ?kpŒëäôÑ?eA°}‡ÔÙ4FGL J0138.5+0300?ãÝO0ÿ@ÀLåùð†nÀ;h¯Á#K_À<¾eò£ +@ "ÆÎ1@^	}?Í[PޔËT?ƒu¤5à?«Þˆ6íg@jÒ/6_¿ïÿÿ" 5•?ïÿþó…õ¿á´ò…Ãù¿¿Ô8ؤ}µ¿êD°~b†ˆ?¶²
>GclUNASNone?ïûúúø?>]GÕ5ó?@Ó´# ?>]GÕ5ø?ïù•82¦/?d¡þpúŽÀ?I«5gG"?d¡þpúŽÄ?ïŸàQÙ?†2÷µ…4?ˆû뉻¬?†2÷µ…5?ïô?ôaùw?N¼È¤""?W€<
s?N¼È¤"4FGL J0139.5-2228¿äô~•üÎ)ÀSˆtÀœ<âÀ;G-½¨l›À=, ñèH@ÃÞ,ñz¬?øõΞ^$y?Ò ì¹ý?ìÜB 6m@"ÿßHÐ@GYþí¿ïÿtõubƒ?ïöû¿©xµ¿Ë¨qx¾¿ÞÇlüÃ¥¿înX}šŠ…¿ïþœÞGžzUNASNone?Ò·NRz?È&±YÜ?æ¤xØÖÂó?È&±YÜ?ᎋqàH?×È©™Â?ÜâéÕ?s?×È©™Â?ÕÆwQœŽÇ?´ªØ'Äõ.?åÄW1¸ž?´ªØ'Äõ.?Öóê­¯€ƒ?ÀãÀ¢µå?ä†
©(?¾?ÀãÀ¢µå4FGL J0140.3+7054?Ò#ÅôžŠ!@ ÔFQóè›À:ÒIì³"À<k{µƒ@!+µg*†'?ûÑòkyÌ?Ϋæã¤T´?Ç3÷©D\{?ôG÷EF[.@ÄøÂôÝ?æ¹úݬC¿é"³ì+6å¿ãËgÝ^ëH¿Ô§ÿê8î¿ÙÓ¡šÀ`¿áP1ZëßUNASNone?ïö©d¨¯Â?MOΑô˜ü?R­6® |Í?MOΑô˜ý?ïñfØý??u¹ðŒê©ù?]2Oþ€j?u¹ðŒê©ù?ヨH?Ãmð »?€Zxíù?8?Ãmð ¹?ïzîlßÆH?xõgqŽW¸?¢2d6þ?xõgqŽWº4FGL J0140.5-4730¿Ð77giÚ²ÀPÞ]öU\À;ÚVùÀ<¦RFñƒ@ªÅZ'§@<Ö!à$˜?Ô4›þxÁ]?Ã6«¸«Ì?è;†ß؝@ðš$W"¿çñ¦¿òÊ¿å…Âýk%=¿ãhN}¼n[¿èãX_<¦¿ïú
!ыù¿ï&Nyà—UNASNone?ïüÉÇi‡Û?>€,¶'Ú
?9±Ä³Á)Â?>€,¶'Ú?ïøÄ>ÆÍ1?gt¬³¬,0?LïäË:Æ?gt¬³¬,0?拉Ÿ˜j‡?…/à'Y8?†Ö˜å^9?…/à'Y8?ïò'уä?NtY±ÿ@Ç?Zú]Þø6ê?NtY±ÿ@Ã4FGL J0142.5+6650¿äŸ[Ÿ1ñs@Ö¬¸ZOÀ:Y§uû.àÀ;nŽ	Bžá@¨³0C"ª@,ʦßi?âä"wy3?âHȐýé¥@¶B9`sÞ@z;×F£R¿êÕb{uA¿Ž oPÅ»¿ç†è‡=vƒ¿ël°Í'Åj¿ç#Ÿ!BðÀ¿ïÿ¥œÝùUNASNone?Ôd¶&í–Ï?ϽÞÞ¾!?åͤì‰4™?ϽÞÞ¾!?Ñsˆ.fâ?Ðî¾<ë?çF;èðLŽ?Ðî¾<ë?×¥¤¾•ûy?¾Ìº"®?ä-- µD?¾Ìº"®?Û)ŒÎÊh?À—	v¢5?âkp9˜šË?À—	v¢54FGL J0144.3+5959¿èw»½¯q¹À"%B{¦À9Ýv<?AÀ;ŒjýŒˆ@:/&‰+¸@ŒÍ{Hu»?ůŸ)üRÌ?³yéûÜ°?ç@#qPM@J')ÞuÂ?恋ñ:j_¿–ƒaô¼ªì¿çÓ¦¹Ù«¿ëg¾Ö¿èR¬?Ž‹I¿ïúK¹ëUNASNone	?ï	*}¢?šÀ>½\á_?œþÚ°]½?šÀ>½\á_?ï›É¨3?£+$€wºÿ?‰
¸ù³6?£+$€wºÿ?ëð§«
¤t?¨:¾Âg?À=aSÕn1?¨:¾Âf?îR> áÃ?•œŠj¥%?ªÜÿãÙ?•œŠj¥%4FGL J0150.4+4848?䶈µ"-À)֊"lXïÀ;•PÔ-êÀ=5²Ñyø@ ÔYM= ?û?ƒ¾f½?Ö19'ò¹?ïöá=@K¡¿	?õ›?¤Á?ïÿFÄ¾¿é9M(¨¿âšýFè?ÎuÎù¢Ãº¿ì
îÛëMÁ¿ðUNASNone3FGL J0149.6+4846?îzÍú"j9?±[ËÀý0f?¨S VÉ\b?±[ËÀý0e?ÍXై"‡?Ó¤2Äý"?è©ÇӝÚÞ?Ó¤2Äý"?ã§ý<èýÕ?·¢Àã?Ø°†.U?·¢Àã?±áJn¼²?¥Ã·
ü?íÃÖ²?j?¥Ã·
ü4FGL J0150.9+1230?î`fFácnÀGè>ÕÀ;LK?™sÀ<‡ñS"ÒŠ@ZEÚ)ו@U×DõÓV?ˆ#›»_?¡»
²›R?×W"%ĵ§@Ù¡œrg¿âg¨mqó¿ß
º¨²ç¿çÜ7Hkª¿ä›…AÚ¿ÑYƒÅœØ¿ïÿ`h¤
UNASNone?ïýÑø¥'D?/—ò":LŠ?1p:Óíݧ?/—ò":L¶?ïþ[ÿé+?IҐ«Ïë?*@oíV°?IҐ«Ïë?ïà²Í?r¤—R-Ëo?oý÷Må3?r¤—R-Ëh?ïýZkÉ?(Žê0Á?3}/ì¡ÃZ?(Žê0Á"4FGL J0153.3+5416?ïþ&•¹šŸÀ	/+f¶À:êo.Œ†À<‹ú©u°@!"6s?þÌœ†³ä?ċÕ`ÅÂ?"oŒ™šµ?ÐGÖ"¶ä-@íîò;œ8¿â'^⎀¿ãvÍòfºI¿äÊÄ°ž™¿ÛþüôâÀ¿âÉUê`o¿Ïu6
GUNASNone?ïÿ…>f*o?~"åÏ·
?°fud™?~"åϵÕ?ïþÖÙý4?Dßñ| Ñ?"'`.̾Ï?Dßñ| Ú?ïöb‡ÔÁé?eçeDaØÂ?S:ðV|-ò?eçeDaؽ?ï÷Àž<x?DUª+Ú?Qè~Ǽ?DUª+Õ4FGL J0154.6+0051¿ïôÜë®bÀMÄq´xBÀ;ÆÙ{0øÆÀ<É·sŸ4
@!³uy/A?ß¡ª	SeÙ?è«@UZ¥h?ïäNÿA"?ü}å#çÆ@†?`"¿áýÞ½ç¿ïÿ<h"?ïÒ¯´ì¿æÖÿöÅě?ÎÌc8°¿ïÍ­ÓïUNASNone?ïÉÄÏÜjK?|7·•8íP?{˜ÊÚ[?|7·•8íO?ïýÞ2}P?ZŒíh?3l~å?ZŒíh?©ÏK¯?™çö™HÇ?¦µcE?™çö™HÈ?ïü¤~¯)?B{aR߸??úÜ
†º=?B{aRß»4FGL J0156.3-2420¿¬THÏ^ïÀRÈÁæ¯ÍÀ:ž¯ñʳÀ<ßŠ>²Ã@&âéê??ý²øE ›?À"8#²â–?ºÆÏãÉé?ünà¾Y"@
kRË)¸¿ïþ¬B鉜?ïû .y¿Öôý"U"¿åv" 'E¿Õ‹¥|§¿ÝªßÃ^UNASNone3FGL J0156.5-2423?ïÿaź?Ù¡ñ+é?ÇH½]¼?Ù¡ñ+é!?ïþ>m=?KVµ
}0
?,&,.çÅ?KVµ
}0?ïÀR'¦X?S^FûY?Öül,Ô?S^FûW?ïþè`bh?Ó§?j©g?'!yùÙiš?Ó§?j©n4FGL J0158.4+1230¿îÜÊ^`û¸ÀG"‹—xW*À:Îû­Šè&À<6Îý(µ+@ÔЯZv@9RKý."?ٔ»#6â?éH#à"å'@øÚ¶š[@O°oó?홽 1xÉ¿çd•ÁGÞf¿ïÿÿ" 5•¿ï5A•Ì…?ïÿÿ>¹ú¿ïÿfb4¨~UNASNone?ïÚà}3?‰ÑˆÔôšL?rôöÁfÁ?‰ÑˆÔôšL?ï¨ ¹ÿL?«µäóiñ?…÷øр-?«µäóiñ?êÜN/Ìç?°0.¼zç?ǘŽÇ@Ì_?°0.¼zè?ïµ5¼Òr?†…eû9ž?'²Ë}#d?†…eû94FGL J0159.0+3313?éÝF"—tOÀ;ÎázûÀ;avؤÀ<¢‡~äâm@ YØ&ÈÙ?ÿ'äÓ?ÇiËu´¸?¶eΐò+?ñÏîTÜÑ'@	Ò¯4‹wî?ïíJÖE¿æ¤œ—zÛh¿Õ°¡]ˆF`¿äÁ—½÷¿À¨W{'ò¿ïÿý¡UûŠUNASNone?ïÿÃw0wœ>ûº°­L>þDgÄ2'{>ûº°­Ln?ïþ¤ŠðV4?EUıÍ1?%·PúœÃÏ?EUıÍ)?ïê¥8À4
?pÎPG¬Ö?eZÇ?Ëô´?pÎPG¬Ô?ïü¿Q»Û?-ÈŽ(n?:Ýr!#˜?-ÈŽ(Š4FGL J0159.8-2234?çXïéɪIÀRv¢‡~äâÀ;ªðÏ
•À<ëžÈ­ƒ[@ ö=@RU?ö•ÉæhE?à»E¼Cé?ïÌýߔO®@» 'V†õ@9A‡´¿»¿îâáH2Ÿ?ïÁí@	ÛK¿ÔäçßCr?Î$Œç¯|/¿èÁèm<C}¿Úˆ\ÛMC*UNASNone?ï²̪º?—͹®på?I½Æj¨Í?—͹®på'?ïu!R?°°F¬Î¯h?'\ûÕ¾â?°°F¬Î¯h?îªâýj¿b?™è—FßÞ??¥QÐ)T	ã?™è—FßÞ>?îƒ~+ßY? HTòÉÆË?§È
B
s? HTòÉÆË4FGL J0202.4+2943¿ì™bð·À>¨
¿v¢õÀ:æëlËvÀ<Œ<´¼4Ï@ϖ‡å<@áa¡Û‡{?Ä¢J˜)¬ø?xÝmÒ¸c?µ·g	úTÅ?þû€'µÊ}?ëUx™]4¿å#¡Å¸¿àwñsuB¢¿ãÉűO˜Å¿Ø˘"Æ£¾¿Ü­Hãs­LUNASNone?ïõõWüQH?KÛ©RìŒù?TP]p
?KÛ©RìŒñ?ïüRyç8à?_?YÒXÐG?=l0Æ8ý"?_?YÒXÐF?ïêÄîD²3?jP΂¦?e;»MÌX?jP΂™?ïà[MA¢ô?ZàæÓU±ª?o¤²¾]g?ZàæÓU±²4FGL J0203.9+8120?ïÏ¥«¾@2ݨG²F9À;"Îñj;À<ª<"¸@ §/"R
?üBöõ•C?ÒN{ãüa?ѳôC‰A³?ýT£
[£•@!ٻ̿ëÍÂ6Ƽ?ïÌ$Ñp |¿ã¬Þ²þE¿Ç=:ˆ'
Y¿äôdUêî ¿ïþߤ?åÉUNASNone?ïþ8ƒ9?1ъ¿ëÀ6?'wΌi?1ъ¿ëÀ9?ï÷zÉiV…?s*
ôÂ*?Q
m-Rõ–?s*
ôÂ)?ïÂÓ]iÔ?{j5
DÙ?~ó–QK
?{j5
Dà?ïÇ7ƒÝGp?kÔ½¡Cî~?|d>\Hs?kÔ½¡Cî€4FGL J0204.7+6656¿Õ,·LÙ@Tâó¾ýÀ9¶ZöƛZÀ;˜í8}@ݪâ`@ؑüí&	?Á °å¹±?Õ›e Á@°Ì¼Õ,?ý0é5_?é²X­@?‹¿Ö\çÙßZ¿äèÈ%ž¿èÚ'Ér¥9¿ïÂ[ßú¦û¿ïþ¼~K	"UNASNone?}žŸ¹z¤?€ÌfւŠñ?ïÄÃÌÀ?€ÌfւŠð?"ößÂ2?¡~XpŸp?ï`Iïvl?¡~XpŸp?¬_õ­Èb¼?œvð»S?î:¥#yÕ?œvð»R?•w]u÷Z?wÙÃ0t.a?ïTEW˜F?wÙÃ0t.a4FGL J0207.2-1832¿â՚8	•±ÀQ¤Þ*Ã")À;5Ç/ÔÙâÀ<ŒN«^½û@C,[}ª@êB¡e@?ÍSW@Ïh¿wêZ½•ì?§{R[Âsƒ?ónÒHaÔ?êšCb«Eé¿éýöHò¿ßƒ3ü†Î¼¿çŽ"'Ùc´¿ÜÜT^ü噿ïîQ Ü"UNASNone?ïí–þ^E
?f
(GÉ9<?bi¡º÷?f
(GÉ9<?ï§2©¬K?šn،	?†3U"ý-D?šn،	?ï?iπÖ?@C±È•?˜Æý%T?@C±È•?ï–ë•gÊ?zºâòö?ŠEº&
…?zºâò÷4FGL J0209.8+2626?ë"ÎN¶†À@›OKD¢À:묊7&À<P{B–~@ÖMô™=@'°Ì¼Õ?Çe¥`ÍX?¥¥
|P™²?Ûe5ŸŸ@†œñû€¿ßDÙ»J¿å$ #!¿æ› ¢ŒÝI¿â}ŠuV¿æcü^ŠÏÒ¿ï×þŽæ¸0UNASNone?ï÷ќÈ÷#?FyjÙ)Ö?P\Æn»¡?FyjÙ)Ã?ïôÿœ÷òF?u£§XÀþJ?VÆv?u£§XÀþJ?ïÓ\f©?s}ð
ӆ?vQôLó+ƒ?s}ð
ӆ?ïæs¼	ã?V£Rǖõå?iŒûCö%?V£Rǖõç4FGL J0211.5+6219?ïª<6dUO?ìXu—5À9vZYê
À;?®ª@ÒÆÛD)@ã.`e›e?Æ$nŸDÿ9?¸½èƒažÖ?íêsÁ˜¼$?þ¾¬Ÿ/Ü?Ôh`;©ú:¿àâíP¿é"@U¿å<jŸ01v¿íEO?ƒM¨¿ïï¶Ü gUNASNone?돛Nô?¾)´MUj)?ýÁ'Çð3?¾)´MUj)?èq£À!D?Òÿ3
X8ø?Î9sÀÿzñ?Òÿ3
X8ø?éèÍFÿF?°‡Ëkê?È\ñÊäí?°‡Ëkê?å|Íèý?µ,ÖdÔè
?ÕâeÐ.?µ,ÖdÔè
4FGL J0215.0-5330¿Íš|׏°qÀM¸H@áqŸÀ;¤†*QbÀ<ër
—@ 
mý´v?@ßËlÂ?ÂF(XcÄK¿À‰¢«'â?ó]]Äuq@ß&–—²¿éS®2­Ò6¿êµ0-Å5)¿áqô¿Zƒ¿×õ·ý‡Õ¢¿Õãm"BJ'¿ïû¥]:ÉUNASNone?ïû¡!ÒºZ?>èüÉNmk?A{xµ—+?>èüÉNmh?ïýza¼Ãç?NFŸO.¼1?4,òàÁþ?NFŸO.¼>?Òrþ?‹âÿMqÑ?ˆc@}?‹âÿMqÕ?ïûS"®?8¾`'mF?C—'±±J&?8¾`'mF%4FGL J0220.1+1155¿çƒ×&h€ÀF´ê¿üÚ²À;Ñù®­'À<̹kÆøw@#£
VE1
?õS"¬¢ŠÚ?Øléã3¬?Ëv远Ž?ñÌI"®P
?üwŠ*ÍB¿ïSIˆà
ò¿ï웟-WQ?å
ë ¢wd?è7¢cl¶â¿Ç,>¼~K¿Ô''>[…bUNASNone?ïý…ô•¯Ñ?-v~yž?3Ð[RtÕ?-v~yÏ?ïýœ"Vyð?Qž¡€TÒ?3ÝL0}{?Qž¡€TÏ?ïÀÏ
Ö¾?€>ÕL[
Ö?·˜z" é?€>ÕL[
Ø?ïû|Jª¤?=6³Ëòl?BÕW•q?=6³ËòT4FGL J0222.7+5016?è%H°j¥À#þ½LýÕÀ:âÓº&×ÛÀ<}œ¸2@ –Æ*œ6@˜Ð`Ö­?È\[öu菿Ÿ.'Û+¬¤?Öì˜ú¸B|@L+Dý?ï÷ýÖÚî¿è!"hýð¿â"ëSÏ¿ãÿëþ@bF?'o¦ß…ꙿê7]>ÊkUNASNone?ïýØäùTn?-g0QHe|?18Ø5\•¿?-g0QHe‡?ïþ×ôR¤V?C¶àóŠÿ‰?"€ºÕº¥á?C¶àóŠÿœ?ïL¼Û?iù—Û´£?aha³C%?iù—Û´¨?ïúÔ:ÉÄ7?7x Eç	?D¯Øï ?7x Eç4FGL J0224.8+2937¿©Ã–­®áÊÀ<ÿÜ&Üã›À:¯Úv»œÀ<I½ò>v]@`+ŽÏ@.ȺïT·?DZ%fìÉ?ª;§\6?à‡f%ÎÆ¢@ajþüu?ÀvD?u
ï¿ëŽèe¯‡B¿âsՅ2à¿êcA¹óê¿å•€¸Í¿ðUNASNone?ïü 7Ø»º?A¢û6ñ7¬?:þA:"32?A¢û6ñ7¸?ïùMÿòX2?lRïú4ù1?JÈ6Ÿ6T?lRïú4ù0?ï²ßDŽqç?N
z/—h?ƒH.Üc…ê?N
z/—g?ïç‡6¡©o?U_ž?hxÉ^V'?U_ž 4FGL J0225.5-5530¿ÚÞ`ÅÍŠÀLvi¾	»kÀ:e'Kí>\À;ÑöÌz—v@‡_/es@°yK!?º!ÿ¯"B¿²ìÈío/?÷t'òÜ+@òÎO§Þ¿èï!áQ>6¿èsшô¿â4¿Ÿè"'¿àJ½ÞYÿäÉGNΚ¿ïøHEéïUNASNone?ïÛ"»ÙX?o~ýÈÅ?rp¶"S?o~ýÈÇ?ï㪘Fê ?"ÃäÛïÙ?lUg¹à??"ÃäÛïÚ?îþ
÷1ÿö?•¢â}9Í?  Œàœ?•¢â}9Í?ï³Ý⅍j?sõK߯"Ñ?ƒ‡^œ¥–?sõK߯"Ñ4FGL J0226.9+7744¿ç€­Ó¬@/©	¾ºÀ;f6䘛mÀ<´ÍǞ@!Muþ‰Þ;?þJÃ")´?Ð_|½@?º}=msËÕ?ïÎùͶט@N‹•‰¿ë°ûœÄ?ïÐâ (z?èF4AÑ¿åá3÷~Q?¿ØáDŽ$p¿áò,}a¢UNASNone?ïü-³ڃ?<xÇcâW?>'gÙ+ì¹?<xÇcâ\?ïøoÖ6Û.?uÂ"‡éÊ?N@§$"Gs?uÂ"‡éÊ?ï¹®¿3.?'DN¬Ùëp?¾TP34j?'DN¬Ùëo?ï´¡XáBÑ?tY³Mâ©Ð?'שǯK–?tY³Mâ©Ð4FGL J0230.3+1713¿ï)±5yøçÀCÉ\ú¬ÙèÀ:a"»ë$À<J›ñ@A€§…?š@ðHðŽ?ÈÿQ™Ð¡?șß9¶Úó?ü8­uïpf@QüïÕ:…¿åNµY+¿á†…‰A]¿æ@O±;`¿æAözE@|¿ïÿ"àT¾ô?ê&f%ÎÇUNASNone?½£}}?¨õ	kˇ?§Öä%È(7?¨õ	kˇ?¤6ÀR?¦‰Eâ†Ü?‹ÓVòOë?¦‰Eâ†Ü?ë:Îu庖?°<|yÓ×?ÃÆ(iª?°<|yÓ×?ïñ_¬ñq?uøÓu?œÔ
aÑö?uøÓu4FGL J0230.4-1140¿ÕNlþAAÀO"[t›À;ãeUÅ.sÀ<åycՒ@"Eñù31?öœªÆÇ©?ݎ½"à¥?ÔÐ&žzT?ù&Ui¾à{@õ•íg¡û¿ï.G P ¿ëÀãàd¯,?ï÷áî-¿ÛW
Ãbó?ʋ)¿A¿â(Ý9+š¸UNASNone?ïüHëMòm?A`ߺ®ö?=¸¥l—c?A`ߺ¯?ïþmÚ~?Ec\ó.xÿ?)"_ˆÑå?Ec\ó.xü?ïÄ­"Ì ?€Cì®ã—¾?}©5™ï·ß?€Cì®ã—À?ïþÏôÎß?!Õzý¨?#³m=?!Õzý}4FGL J0231.0+3505?ìAdiðêÇÀ7wÂôÀ;¥`úÛ4À<ÓW,6¿°@!õ¸¢žP
?ÝáÓD59?æ¿qdÇ)ö?ïÿ¯Èe_@SÞ|!¹Ž@‰\N4–`?î`pî¤ü¿ì¶´ÝlØ¿êނ׶4Û?䗖ºÖ*¿Ô:睸0¿è'#ᆘ5UNASNone?ïܯ¥˜1¼?qËÜ vxÏ?q¨-3ç"?qËÜ vxÍ?ïîÌ	Ÿ£?',ÑÀpå?a3ÿö`]ú?',ÑÀpæ?ï(
Zy9þ?'ßñèŽêé?šþT°ØÀD?'ßñèŽêë?ïß&-³¬±?s"a±0?plé&)§º?s"a±14FGL J0235.3+5650?ÄPw¥ïŒþÀ	ŽØ'ãt¯À9­Ž»ð·À;§³Æk‰¼@Š^nJ`v@Ð >cé?Àã[š£~?×êÁªYÛ>@¦Ñµ(k@KªûìŸü¿ÓÌŸóOî¿ÀùÖZÀ¿çA>U¦%¿êœ}ÿà¿ìèÓ=ª/"¿ïÿæÀ
UNASNone3FGL J0235.7+5647?£f}Ǎ?µæ"1™z?îɞ8#‡/?µæ"1™z?֒O"+¶œ?ÒîÓ Êcž?ä¶Ønê$²?ÒîÓ Êcž?È`Æ㱦?±Òʛ`{?éçÎG–`?±Òʛ`z?Óa†áWŠ5?­?¾ÑP"?æO<T:ä?­?¾ÑP#4FGL J0237.8+5238?êyHL˃ÈÀ®–ÃüC³À9ÅÛ_6Ç<À<VÁ1Ž…@Vá:B.?üèM&#€8?¾ÎG*`ý?㎧Þ*î@ tNrSÚs@T	|€"¿©q¬]f–¿Î÷çؖڿˮ)7'¿ã®T§!A™¿ïÓ4*…¿ïÛgNnUNASNone3FGL J0238.0+5237?WK‹,¦vZ?S'qL²?ïôZ:i¬Å?S'qL±?†ôô')>í?áêٖ{?ï¤,-÷[?áêٖ{?‰u€öÓÊ?oÛD3‰?ïš)ü$°Ø?oÛD3—?hŠhEÊ…?Y)B)Ê
?ïçu—ºp5?Y)B)Ê4FGL J0238.1-2621¿ìՏÁúu	ÀPŒ¢3œ¿À;쪸¥ÎÀ<°䭔"@"³Ä=1@"Ã9¦?ċšþôg¿Š·t˜O¹ô?Ãþ$@­š@
93Ù?ڋւ®°¿ê3*š}£¿ã›¸øÚqÑ¿ç¼àáVǍ¿ãÁ2d×.¿ìÚ¡oBUNASNone?ïþòºL ?ô¿|õi=? Þ$[>
?ô¿|õi
?ïþ : X?C;¡"ò³½?%ü]÷*xt?C;¡"ò³¿?ïèoÙ`)?eWµ›	?gp&ŸÖT?eWµšý?ïÿ7ÊSÚ?|_.q7M?9µ"Çý?|_.q6Ü4FGL J0239.1+6634?Ă9õ"6h@¦¨¸ñM¶À:!¦+xSÏÀ;¦åßÃI–@K|¯Óí¨@îOá¿£?ËV¢ùê'0?Ì2#(N'Ö@¢]<ñøÖ?ñ
4EHß¿ïþ] o!?ïþ¿Þ§À¤¿çËxÎø¿ã#9 µ—§¿ì¼¦¿Fý@¿ïï–áXuUNASNone?♇Ï݄…?͍ëþj?ÚÌð`Döø?͍ëþj?ÜóÅ¡>Å?Õ¬_"Ît?á÷†/`?Õ¬_"Ît?á?N㑟?¼FD"Ms?݁cÊ8ÜÅ?¼FD"Ms?Ǝéå:I^?°Ó–mLÈ?ê\E†±m¨?°Ó–mLÉ4FGL J0240.2-0248?ÈùMÙÉ1gÀK1ÿ`Ï‰À:Ïú÷''ýÀ<{q°F"I@ýw:Ê@g&Š®D?¦‡h¿‡¿‡*[?¹ ?Ã@ŸØMœ@òïÌ+<?ãº4¿O`»¿ê{ù?ò^W¿çAÿI ÛB¿ç1‡+ØË߿ҟhûìõâ¿ïþú·ŠñUNASNone3FGL J0240.0-0253?ïþ%£àÕ?*
Ãx&vv?.­¥Áò©¶?*
Ãx&v_?ïþuvè]Õ?E*8n8zú?(¨'z"°?E*8n8{?ïê·¿g¤?f 4È?eH@˜[ñª?f 4¾?ïþ[CƝ?!&ÃCÊR?.šKÖ1?!&ÃCÊ!4FGL J0245.0+4755¿ì(;þ—öÀ%vbwÄ\¼À;õ5¾À<X;ãv@1ˆc;d@+­Ûoý¿?Ƈ%£¨'.¿˜Q§E1k?ËƟ¡›p´@ˆH®ðn¿ð?ïÿÿ^ðP`¿åMv«Xÿ¿é'öè)J¿Û­"\›Œ¿á2ÚþhÑ%UNASNone3FGL J0244.4+4745?ïüÂz4ÜÏ?EÑZ+W°ã?9ì.YŒ?EÑZ+W°è?ïþ0"æ¼Ù?QÁÏ.bë"?,ýє2m:?QÁÏ.bë#?ïOJ)šÉ?'æT@þ?–¶ºÌ¦ç?'æT@ü?ïõj{n|}?Háû½aÓ?U+	#?Háû½aÙ4FGL J0246.0-4838?ãåêmJÀM£~õ©eÀ;(×å.ÃbÀ<h¨-±@ç×õÊÇå@µî;²]¶?Äç©Ý^•b¿ºHY`™?òI²Çh	@ˆú:U¿çO¶@ï3¿éG¿å‹<¨&û¿åJæþ§:l¿ïÿýF\I?ïÑ6‰)	UNASNone?ïü¼fÂr?FbÌ;ù‰??Éìw?FbÌ;ù'?ïÉêZދ×?¸ZhKŒ‹?{
Ґº{?¸ZhKŒŒ?ï³cñ'¹?ryÆp*Ó?ƒ'›Qº%?ryÆp*Ó?ïîXH۟?X'è¶d6K?a§·ÿ$`Á?X'è¶d6R4FGL J0251.1-1830?åcy­€¹¦ÀN—ñ{ؾsÀ:öbWãì¤À<pD5¹ö0@!vfóT ?ôç"øoé?Ñ8՟eæ?Ü_õ~F×Ö@Ò¯dÜùk@7µ	Œ›¯?ï0ÒÐòÌ;¿î×Û'Ùc?éätSŽóM?•Q:]³¿Ñƒ˜{au;¿ãáý`"iUNASNone3FGL J0251.1-1829?ïWCV
^m?•€¡"žC"?••>T2s?•€¡"žC"?ïátGEÍ?šc6…À ?nꋸº4)?šc6…À ?ìI 7`?«S¥hÅÂ?½²ÿ¦Dÿå?«S¥hÅÂ?ïh#¤4ˆ%?Z¦£q¾?'û‹ynûe?Z¦£q¾4FGL J0251.6+0628?Áÿ\ÿ(ÀFÉD€bïÀ: ­‹¾åƒÀ<'¤ˆ
%@2au»Ä@ZYÀe¶=?ÄûZiXU?¨«œÀ.rž?á—ÈAíá@ópOžN¿ïn'>´Ï?ì'VÃ[4¿í?Í«Þ¿Ú4çhY…­¿ì_Ïsp:?ѝV}JKUNASNone?ïn}ßiÉ7?˜G,B©Ð?'0DÆÙ?˜G,B©Ð
?ïéP/¹~?ƦíßãÈ?f¯~ÐF'?ƦíßãÉ?î›\FƒÆ¼?™`3 z÷?¦J;—Ô0?™`3 zö?ïã&]âÒ(?aO'ÉK N?lÙ¢-Øu?aO'ÉK M4FGL J0252.0-3657¿ï!ÁßHlÀO`˜²é̸À;ŒôNÀ<꬇²çH@ :¬þT?÷ó朁«f?áHÌ!¬"?ÒMÝC¢•?ò+Z;µ¸´@jOøË¿ïüùOâ–c?ïÈNòÄ®¿èEr/ÈD¨?'{o"i©¿æ~râÅB¿ïëá/Z`ŸUNASNone?ïÿu%
¹Ï?6IÖN¨¶?[^HÆ?6IÖN¨H?ïþ
o›{?P˜|áÈ?/)F(Zž?P˜|áÏ?ïÆ®òMf?}[³kÎO?|¨†ÙuÍ
?}[³kÎN?ïý?ŒOo`?1•`#çÈ­?6""øž?1•`#çȝ4FGL J0252.3-2707?ï÷72G,ÀO•[0HÀ:Þ\î 0À<¤¯¸k@…kûü4@x¦f0·?ļÚçB¿¨DŸ[f?Û$[)'=@æ"B€¿Ãø*ÞûÎm¿êWådsG¿ëˆ{¯£Ç¿ãýBJþ+¿àvžÝ¦8ä¿ïÿÒkÀUNASNone?ïÿÅË[Cé?ú{ås>ýR^Gè?ú{å"?ïù"M¤q?gÁ‡¯eŝ?I²Én:?gÁ‡¯eś?ïÚd?üH?vçÏ\ªè?rÍàuÜH?vçÏ\ªæ?ïþS}/†s?"Ò%Eg?*È-˜Ó%?"Ò%Eg4FGL J0256.2-0408?ÀS~º#£ÀJ2ýX…ÓÀ;Wy{ ÔÀ<²°9ï@ »Ûۈ?ÿª÷	º?Ó÷e<DÔÆ?¯i³í'Ð?܆p|¿Ä&@GBW=?ïضDË,¿æ
¨ÐnB¿ålKîñ¿Ôè™Fƒ¿ÞZZT	l¿î.R¬,ÄUNASNone?ïÿÙ]Ñà?>ñÄì#S'ª>óQà'T>ñÄì#S&¥?ïþ†'WÅ?DÒ\íÃ\™?'—Úƒ¯©?DÒ\íÃ\"?ïø.W'
?]îK-j=õ?OGþ¡·ÍÍ?]îK-j=û?ïýÓ2h?"46[ðF?1gŸfl¸%?"46[ð?4FGL J0257.8+7044?ܶ–fk€›@$ËYWŠ*'À:6ÄÂ<PÀ;Áœ¸2@»	sq@N`›KJ?Ä̎c…‹p?°ˆ›ÅmÝÔ?ç?	ËZÜÅ@~Ñ{]A?ïï;At"|¿ár%acr@¿æ,æ³'à¿è¬ôŸú†Ä¿çrSÚr§½¿â€fWLíïUNASNone?匿ïdƒ?ƒ ;)‰"j?†&ß<!?ƒ ;)‰"i?î,)uÓé
?½½7Ýí«Í?­=h¢Áoj?½½7Ýí«Î?îT0˜m1?œíÝ<?ª¼öy,æø?œíÝ:?î'"Þr?'Å@NÈ?¯Ö²á?'Å@NÈ4FGL J0259.0+0552?ÜàvGgÞÀFiÕ^kÆ"À9Ìü}"€UÀ;êêÏS)@˜{RÜ8?ýì}6Œ"?º–R<bÜÄ?ÁÔDe_«6@Xî¼
ݪ@	(±‡w@¿ï¶öÁèÃ"?ëX½0w—¿Ý{>ÊÁ¿ØV«ùµä¿ä÷9½ï§¿ì×B4ÍgUNASNone3FGL J0258.9+0552?ïócª¬Œ?[|þeO?Y8ª§Äçž?[|þeP?ïöíÊ$7?sÉFó[?R$kõ·"?sÉFó\?ïŽÿHg!?ˆÝ¥ËÛ?Œ@>mæ7Û?ˆÝ¥ËÛ?ï¨vؐ';?uºh›ùˆ…?…âIÛÛq?uºh›ùˆ†4FGL J0300.0-5908?è2}'ÿýLÀIˆõn¬†À;¶,c5Y~À=™'óe@ 8ÅßÉ?÷Ũ›•\?ãp"'0Fo?ÛÀ?øzDàÑ@hÀà?áÒ¹Ág‰¿çâ,Rƒ[¿âü»§á[¿Ì!ðj¶­&¿àÏà}ƒ¹^¿ïÿ‡4<G¯UNASNone?ï÷®")9+?Neg	›?P£»­©€?Neg	‡?ïýƒ‰»#?Rù8D ?7[ã²&å…?Rù8DŸ?ïµþ[oes?ƒÖLÇÖó?'€i$&£^?ƒÖLÇÖõ?ïòêô›d?Pd"plo?Z*É6ý÷?Pd"plo4FGL J0300.4+3450?ïԌK‹|'À4ìûTŸ"…À:Þ½Ÿ¤vÀ<X®^L¼@pâ²gEß@—XA	µ‹?Ѻˆ¼ývä?Ïg¼&âAÿ?ö	Ã}˜²@…¼:…@?ïæ|Öë3À¿æeÔp/=¿Þ*t]J¿é\#ý`='¿ïÿü¥¬¨?ïH±(UNASNone?ï÷õuT?Xµm(úr'?QøáX{?Xµm(úr%?ïJ-Vôð?¤t'ƒ?–ºU.Ab!?¤t'ƒ?íÂþqb×?¢ùS"i?·áètéH?¢ùS"i?î<åÄDÐ
?›JU,b?¬1£»²ÿf?›JU,b4FGL J0301.6-5617¿ïà
½¸ÆÀJZæ[ê¢À;ŒAÀ<ÐRì6 @ 4±âe»F?û˜ç<º›r?ȗ…4²º?ÊU»Gi@½&fœL@ŸØRg?éÏYoØ¿èBã_5o£¿ÑÈ¡jÉM¿ä9[€Ú0
?£¢y^ˆ	¿ïÿÿÊPËUNASNone?ïþfÿԀ?(¿¯E³ª?)·þê?(¿¯E´?ïýßÐÕòõ?Ls"Ô+Ë?1yPhVÙ?Ls"Ô+Ë?ïŠìþ_?‡ºzÇÀcB?DÀ|h9Ë?‡ºzÇÀcD?ïùE.d1z?AD'x6>?JëFo:?AD'x694FGL J0302.5+3354?á½ñ狑À5…aܓêÀ;!?8$4À<çÈі@!î>tÎ?ýìEz]"?Ë
¯–:|?˜P|Å"‰m?Ðå³£†Œ@9°â‹{?é ð‹C¿ïÔJ«þ?í]@þ"b¿Ý¨áá¿ÝÂ)ÜÓ¿ÔñÌËö
8UNASNone?ïÿ'!vÁd?87¦Z6?w¢O§b?87¦Z6¼?ïþR›û‹^?W`'ã¾îF?*Ö@GJ7?W`'ã¾îN?ïûu7[²?JªòJ
; ?B+#š'7I?JªòJ
;J?ïùNû÷W?@ù¸Ä 6W?JÄ#ö¡N?@ù¸Ä 6N4FGL J0302.7+5717¿Åøì[ç¿òÅ
 ÒrÿÀ9¦é#D¨¦À;@«‡ça@'î
_)†@Gá%Ie¥?Æb Â2À?±Ô9}¥Z?çˆÜä.?ýE´ÒÛÇ?îïsàøRâ¿Ø\&$p¿è¾ne8¿é 6Ff—¿ïç"=ç¿ïÿÚÁ,/´UNASNone?ï•y`ôš?•»qÆ<9G?Š¡¸§Âك?•»qÆ<9G?îJÂÉÔ&?¼­Ûæ¨ix?«Sޓb½¨?¼­Ûæ¨iw?ëhÎ3ô|#?¨weäñ?Â\Ç0.w?¨weäñ?é]Úñ°?°ÃéíQ¸?ʈ"9?ƒà?°ÃéíQ¸4FGL J0304.6+6554¿äh=*Å@Ü ~$É
À;CY7©ºyÀ<Ç
GžÑ@Üv¸îô?þc\ƪt?Ô|_p#?èç~>tYï@
‹(Øf^@Ê.¸Ð¿ïüÿÐ/WÜ?ïtÿ†]?Û‡!F÷‹¿àÓöAC/¿í«ŽÄS‡¿ïò 
¼%UNASNone?æô"Á6ä?ÂÁò)IJ3?ÒÙÌ}'8?ÂÁò)IJ3?ß2æþï°?ÖW,ˆ™ê?àfŒñ€ˆ(?ÖW,ˆ™ê?åçc'ð'Û?¸†±´?Ô18ÜúJ?¸†±´?ÔᓃqÀÛ?µ‰½eèö?å6>G'?µ‰½eèö4FGL J0308.9-4702?ßEÉW@7XÀLDõýG¾ÛÀ<U¾š#À=,jËOõ@"ókò¬?³‰–íï0?ì(ót'Ý?ïÿo¾ÁÇ@FÍ)Á@,xËëÚ¿ïûÁa´¥å?éßð•ÿ±?ï--àôË¿ÚJ
Dý`?Þæ3:¿ïo¿ïÿñò÷UNASNone?ïí™ÍÖò\? 4–vñá‹?bf2)
¤°? 4–vñáŠ?ïýS­‰êž?bó°ï2õ?5b"°«%?bó°ï2õ?ïuÞ՗×?"z`:ÆU?œ'D%MD?"z`:ÆU€?ïÿkˆ['N?g
¹¤L•?ŽôÖK®?g
¹¤L®4FGL J0309.9-6941¿Ä2¤ÁY	§ÀE}Þ?»×²À;S'¢xæÀ<ºôúé?Ê@u~5ºø?øÎrýMž?Ûh«î/ô?îº@ãÉ@Û¼¾aÐ?øì–ց?ï£^>y¸S¿éŒþ–Ž¿ØWæ'öÀ¿éÍΟµ½g¿ï`Ÿ¨žð¿îs´ÈUNASNone?ïÍÄÊH'\?€.#OD?yšÛ·QÁ?€.#OC?í$¾âIV%?Ɓvø¹(~?¶ÚíµNá?Ɓvø¹(~?í!ˆèG?¡¤ôÙVù?¶ó¸½Ç/"?¡¤ôÙVù?æØc'N
?¿i4q_s ?ÒOû8ûcå?¿i4q_s 4FGL J0311.3+2940?ÝL^ÒAÆÀ8}E¥ü~À:"å~tz%À<EuU³@Ê®ž8¾@µ¼D¿L²?Ò³A Ùß?â-Ánʸö@	m‰‹.œË@´0©kۿك#€¸¢¿à(ýOK˜¿é3eÞPÞ¿íšÿZc¿ïø`ˆ"?îÜÔ·|ÙoUNASNone?ìÝB|u?½aƒü©þÕ?¹ì$T?½aƒü©þÖ?ê­\³	Ñ?ϯ F¦?ÇõJ3ؾ?ϯ F¦?æVeÁ—§w?µ®qk×Ç?ÓS4|б?µ®qk×Ç?äp<i3ã?¾ì‡LG?×χ-˜7?¾ì‡LG4FGL J0312.7+2012?åå¡ô
£À?"›«–òÀ:ý=1¹¶pÀ<xŠ§ŽNã@!²ŒÙÔ?û/ä^¹É»?ϞîؐOn?Ä&܍µ
?øI¢@1Hw@o˜Njò?Ûª%?éÌ"C>C¿àMLïœÛm¿¨c¦¬D¿æ¤ ù¿×¾ ºKUNASNone3FGL J0312.7+2011?ïý¸4h?.	ėóðú?2>\»ÎÛ?.	ėóñ?ïýßðWŒ?Néü¦5!£?1}CŸÀ?Néü¦5!–?ïãP~j?r®	Î1~Ž?l¯áþ–y?r®	Î1~‹?ïï4	½®?R" µà†?`ËöïBRM?R" µà}4FGL J0313.6-7508¿î踱CŠÀCd0 ±»ÏÀ:Äs'ÈÀ<n
Jk^@W)ªs[—@©L_T#n?Èôc>¾¬¤?…sÐ -5Ý?¸ñ›8U1
?úoÒ@):â¿æLœ[ùŒ¿æçeÕFîÒ¿ë"–Þ(i׿ê+ÿ,›i}¿ïÿå"m/®?ïný
Ý8UUNASNone?ïÿ<lªC5?$Lø4«0?rj·™Fž?$Lø4«0É?ï…)Îñ.`?£P‰E|ŒP?ŽµŒC´h ?£P‰E|ŒP?ïk)çg®?‹Aœj?'šÎC
<?‹Aœk?ïÀ)œEûF?vðnkv;?ë1Ý]‹?vðnkv;4FGL J0314.1+2827?ï$*‡(ÌÀ8ºH×à&FÀ:•…ú€d>À<³ûD¯\@éeSi´@_yŸÿh?Ë/¥õrˆ^?À¬°Í'Åj?õ?|Ì@Sp?íf'•ù?ÉYF˜?ÒS¿ìr9}û•¿ÙUkÙ3¿áa?èÅQ¿ïýç¡åBUNASNone?ï¡êÀàu?Žú«ðÎÀ?‡½OÇã?Žú«ðÎÁ?}ñÄê?¡˜Žwuˆv?‹ ƒŽÅ]?¡˜Žwuˆv?íÅcõ5?¥DéÖÝè?±ÔàVW×Â?¥DéÖÝç?î÷œ± ®?ŒÜ¹O? †4åþ•#?ŒÜ¹O4FGL J0314.1+5033?î"d'îŒÜÀ—
€Œ'ZÀ:$²øæ0KÀ;È5"_õ@c«¡@¯X}o—h?Íé>]ˆÇ?ÓÒT`ªdÃ@ÉÅ!Ý @¥9Œ=»w?ÔZÙa?ïꧾ d9¿çZ"zy¿äà'÷–¤ó¿ð?ïÿR[§UNASNone	?í¨¢ÊSî'?¶ƒY[~yT?²ºé­`ŽÍ?¶ƒY[~yS?ìí
ÔÚ¹É?Äâ4«ÃyÏ?¸—©Y*1Á?Äâ4«ÃyÏ?ãëžÌ¬Ÿb?¶­âN1i?Ø(Âf¦Á;?¶­âN1i?ìH
u«qN?¬FÝky#‡?½¿¬R¤u?¬FÝky#‡4FGL J0314.4-4805¿ßún§
ÀK¡cÃ÷bÀ;NüÕ©À<èŠF?@çÖA•¡'@ ê@{S?ˁ.(\j?¶Â\ÜNõÜ?ë²_~ØÕ@–É—
MF¿êm§¾Šà¿Ç­¹v®³¿äömŸë˜?¿ÜÂ=|¸7¿åÿ‰b"ʨ¿ïÿýF\IUNASNone?ïýç‡zTr?,oî½·i?0ÃÄ-\u‡?,oî½·i)?ïøL"ûü‹?jØ^®••µ?NÍì
Ò)?jØ^®••´?ïÚC?ç?shÕ>¦ü?rÞ|à{Œf?shÕ>¦ü?ï牬¢pá?Wö3à3?hvS]å?Wö3à34FGL J0318.8+2848?ã$Éö'ƒÀ7×UÿæՍÀ;)-c™ÑÀ<¿¹üæp@)Ç`|B@Á#>?Ù	E#¿¹?ïáµA•Ì…@ë¬c ¹I?ÿ'ž=BU»¿ãLYàF&U¿áãùÚLQ¿¯üòü®´*¿éíô?,­¿ïÿ\ è,û¿Ëƒ–¸h¼­UNASNone	?ßÉÿDLÐ?Ìóì«Ãp"?à|Ýٙ?Ìóì«Ãp"?ÞwR?և;9•™¯?àöDryÖÿ?և;9•™¯?Üæ§Áz?»d²‹¶*J?ጬ|{Ã?»d²‹¶*I?º.¿×€{ª?¦'>‰?ìº(ð‹?¦'>‰4FGL J0327.6+2620¿Û O	?Ä«À8¦°úß.ÏÀ;E'ømd‡À<—ªÉlÆ@!B`E:?üž×¬#ßÙ?áò_£Ô†?»ãâ½úÌå?ãe	ÚtU<@éBb{[?î'ϝ+õ¿èWrþ$]­¿ìJ-J»æ?Óºí¡Ç¿Õ yó$÷¿áâ"I΀+UNASNone?ïÿ¶Løã?!_¦1_r?	6`ã"9?!_¦1_|?ïýð)F'Å?Ufõ7 Í?0~µËià–?Ufõ7 Ó?ïž5Š•è?'Aî«7?ˆr¾Z…¼?'Aî«7?ïö';?J{½Qæçb?SÿÏö݉Ó?J{½Qæçk4FGL J0328.4-4736?ï—3/ÀJ¢s-õÑÀ:ƒ®E"IÀ<µ÷ڗ«@b±½|ͱ@¨¿§J\?¸ÚÇ6_ãj?"O®ÐËS?Êß«6Os@´Íí^<Ì?Ñ£ø'Äj¿âõmÕÆp'¿ça"oŽ-¿â¿§µ¼¿àá:þϾ¿ïÿþR€ÖTUNASNone?ïÿ )Ñ"?ßÀ2x?úÅß¾4?ßÀ2k?ïþq˜¤.h?F/ö³8°G?(æu½ˆ=?F/ö³8°<?ïðpUv&¬?d*bésˆ?_U²©‡?d*bés?ïý•4»ZÅ?#Õ†=Î?3VZ%)ۅ?#Õ†=º4FGL J0328.5+6114¿é0enqàk@`'ßBñÀ9¼.±Ä2ÊÀ;wÕ<ÝÖà@¼®'úï@í`Á
ø?ÇV–$D-?ËÕü3Ã@B`Û*±@ÂÅ(=¶Å¿á¥‡
¥Úð¿·<Ê5ñE¿éÈ>O¿çÁ‰¢«'¿íÒEb	àT¿ï©œQ3¤UNASNone3FGL J0332.4+6110?Ïf²¨®DÃ?ÉÄ?9à¯ñ?è&SUÔnÐ?ÉÄ?9à¯ñ?à?y´öny?Ô.R>%ñ?߁–#
?Ô.R>%ñ?ßÃ_WŽ?¾ãìîÒO{?àPTsü9?¾ãìîÒO|?èI
.@´?±2
hn?ϺÛ×Fý0?±2
hn4FGL J0328.6-1129¿ï‹]vj*MÀHü«`kz¢À:Òe1³sÀ<"½	á*R@ONœÆ@)ÑÀQ"G?÷:ÿ°Nè?'–¶q2?ϱ^œÃo¬@e-a4l?Ï´UªV€¿è—ñXP¿æ?ªºÔ¿Þ墜!´0¿éÙßÚƋ?ÑZ½:ÞxUNASNone?ïðñnfº?XAa—_&?_Î#2‹}?XAa—_&?ïû—Ê9­\?[ñâaoö™?A ×JÁ?[ñâaoöœ?ï̚ué…X?}(æ^ŠŒð?y²Å=SÍ?}(æ^ŠŒñ?ïñŸýµ<?L&"êŠ{?\À"Ňì?L&"êŠy4FGL J0330.1+5038¿ç'"ôºƒÀÉHýŸÓÀ:!2m:•þÀ<º«bú@Ó4E@äÀ§$?ÄBصä(?Øü;Ú÷‡á@n¡žJÙB@Ú²šF'¶¿Ù²^ç0¦¿Ö¥›E]à¿ãí¿@r5ý¿ã•#þŒãS¿í«&[´\¿ïµëÿíáoUNASNone?~2½'d?|‡çêk°Ö?ïڅðÝÓ?|‡çêk°Ö?ÕfSÂvÖÏ?ҏAæJ3Þ?åLÖĔ˜?ҏAæJ3Þ?¥!¡gûÙ?–=3y¼Ü?î­å懲C?–=3y¼Ý?ћ3p22Ý?®xS©gq?ç2fGææ'?®xS©gq4FGL J0330.7+5845¿áâåy1â@-Í9ÚÀ9wb§•À;4ž"ºåD@~B¨œ@a¤_Æ9?ȈªÉlÅü?Ýøk¡Ž°‡@h£?4É@3:·áÙ#¿à6€d¿§ŸÑþ =¿åÔÀdïn¿ï6ci[ä,¿í"äEV¿ïÿç<t%UNASNone?Á€"¸.àê?ÃÌ¡iÇ?ëŸÛôGÅ?ÃÌ¡iÇ?°­È¨óµ?Á?	c*UK?íêFêüÁ‰?Á?	c*UK?Ê2•ü?²S K(;?észš€û?²S K(:?¤]S>
º?ŠixL·Ý?îº*Ì_Å?ŠixL·Ý4FGL J0333.0-3044¿èPQÞ³öbÀKRxá"-oÀ;MœÏڞÀ<Ø´*>—ë@FdV@Ô\?ÿ«[˜­
?ÇSÀÜԁÍ?ªhm&ÉîK?äÏ Ä0@©CU,¿í¦M;òõV?ïýR¦–_¿á:ª‹Ydö¿àH?xæò¿ç/jñæaÉ¿Öф!bPWUNASNone?ïÿ_¿ßö?fr0\ºÛ?Aª?fr0\» ?ïþ2·7•ç?N]#®u¾?,Ԍ†¡}Å?N]#®u¾?ïíÓ70Üñ?ed~µo'?b,ÈÏ#Ë?ed~µo"?ïý)1?-{Ö¦/‰?7o^·.x:?-{Ö¦/¡4FGL J0333.4-2705¿éªÓ>œ6'ÀK¶"‹ë[À;=`ðà:À<Øꭈcç@K¼À('?ÿÆü9¡â?Ê}v"q?®†‡™'?äh][Œ@ôôÕ)"¿ïŽÄ¾áQ¿?íôÝ!®¦q¿ç <4cµ¿Ä{ÿÀ?пåÝÞ!ÞÌÿ¿âÆV@~uQUNASNone?ïýk¬Õà?3<­Ö³?4¢ŸáPü¢?3<­Öˆ?ïü'®æn?Z«Ñˆx?;j‹Ì'b?Z«Ñˆx?ïî7ú¼cž?d÷%¤¶!i?aÈCœaÅ?d÷%¤¶!^?ïôœó	(?JyB×jC?VÆÝí°=?JyB×jB4FGL J0336.0+7502?Úö NDJ@/DêÀ9ŸÏ!:ã+À<Y›0r@\kæ­ô?ütàaÕ.?¹	àÔk§™?ُ/Þ?@ 	ó蚈­@LŽ\¤œ?á%âØo˜¿ß¬übf§¿ÒQþ$ˆ x¿áQ"²ªØ¿í*ÎuCxü¿ïý/k'–GUNASNone3FGL J0336.1+7500?i¥\›Øï(?bèv
'NÅ?ïæZ£d'?bèv
'NÅ?åÃ,ë?Š÷^Upçe?ïÀ4y¦)Þ?Š÷^Upçe?–
P
?Ü3ØÝ]?ïO—?Ü3ØÝ]€?Šqî^\?xiüZŠDá?ï–;ŒEú‡?xiüZŠDá4FGL J0337.5+2423c?Ô;¼8yÅÙÀ8½ëcÉÀ:¨—,ÊÀ<E»,'X'@#:´†ÚÐ@"WæpâÁ?Ç}–™4?Áo,ž¯N?öŽÞ9ܚ @(Àr×
?ïï"b*—ƒ¿Ù£`rpá¿åSj
_Õ¿æzˆ\Zsê¿áåO_¹£û¿èӎg.UNASNone!?ïçþk€õ?i€äåÆÜ?h"
s…?i€äåÆÜ?ïû—9¤Û?ZŸÕu‹û†?A£m¼•9?ZŸÕu‹ûˆ?﫨h5Ÿ×?'±³0A­?…åò˜
?'±³0A­?ï¶xb§º?iâîfÁ?'açV;''?iâîfÀ4FGL J0340.4+5302¿äÐDÐпý&^ê–À7½?R%gÀ:ÂÊC…Î@ŽÛö¶U<@Àìœuìì?°¸q`•l
?äéÝ~Ë·ú@*Q)®O3@ÆÂûè™1¿½2t†¿ãˆnßßh¿í³k¢Š¿ï"Ú'—õU¿ïþT~ÝU±¿îmõa™šUNASNone3FGL J0340.4+5302?ëf8qÓÿ\?ϯj%¬f?Âg8°"?ϯj%¬f?th8KƗP? é[Œ¨˜º?ï×/hrÑ? é[Œ¨˜º?Û
öCZ…+?ÁÄЧiÞh?âyÞR½j?ÁÄЧiÞi>¨î:$õÃ>¦Óï‰>PR?ïÿþq_>¦Óï‰>PR4FGL J0341.9+3153c¿ïÿúþ	Ú¢À2]`—ÌÀ:4NƒÒÀ;mœzª@/¿@÷C[Ÿc?ԞLœ:Þ£?ÜÏí]æåþ@âyWòÔ@\ò´½âN?å¹ÛÃà•?ÜÙ&wc
ì¿Ù5ä=Àµ¿åÄîs¿ïýà€ˆÑu?ï©ïÝÈóyUNASNone3FGL J0342.3+3148c ?Õ¡gDAQ:?ʸâtÜ?å/L]ßWb?ʸâtÜ?ä•×ýŒ[?Ók‹õãd÷?ÖÔPçIß?Ók‹õãdö?Ô·PS§²?·p¶ýçÃ?å¤W±V,'?·p¶ýçÃ?âî\o?¼q
jÕ?Ú#áGËÑ"?¼q
jÕ4FGL J0342.4+3125c¿í…)Üd	ÁÀ2©Åæÿ}úÀ:Õ@8ÕÀ;x=õ.æ@N‹Ô4@J·'$1?ç&
{ÅÕ?Á6fC€Þ7?û6jŠ¸UG?î`
­¿&­¿Û›ã`bt¿ãôw JŽ¿éÙȓ'(d¿è«Ë*5]°¿ÐÝg#Д­¿ïóy^æ•KUNASNone ?îu¤S["?³l¤Gf{Ð?¨¥ºÊMÞ?³l¤Gf{Ï?ì¨:ÿ-Ç%?Æ^+¯Û"Q?º¾('ÆÛ?Æ^+¯Û"Q?éÃ'PÎ7?±1mO?Èóݺ¼Ç$?±1mP?åŸîU‹?ÃI*Î8ˆb?ÕÞÀ#Téç?ÃI*Î8ˆb4FGL J0343.3-6303?æ½ì$zÎÏÀFF	=–c"À:Ÿ–€	¥›À<¬F<$s}@Á²2l¹½@b°~¸lÃ?¿Ù•2+Ì7?©wDã'i­?ë™þ^?Px@¨S¢ivç?îg‡=¡v2¿çÍMZü¥Ø¿ßçÚ$#JÞ¿ä~q f¿Úiœ;_|'¿ãTÝ<†™UNASNone?ïò»†ƒN?Våþ~ÍQ?Z‰òùfÐ?Våþ~ÍQ?ïûer(«?W=¹U?Bj7]Sæo?W=¹]?ïå¹´l?qÿ¶$«Í?jFK"ïùÍ?qÿ¶$«Í?ï؍† L®?`€Vºõ ?s¹<¯Ù¨ß?`€Vºõ4FGL J0346.2+3235c¿îÌ`"
0ÜÀ1?&9O¬æÀ9ç"gnÀ;ˆ®¬Ÿ0@À}ÆC@FÃ1B˜?Ë=+¯†?Êr)H!@Y)Ù‰t@«;[ º ?î/ŠÂ;N`¿Û!ª	SeÙ¿êÜÕÃìS{¿æàáVÈ¿ê3Òê¿ïq"L["fUNASNone0?ë#zb"=?ÁùY¯*_?Ãr²uï
?ÁùY¯*`?ìÎ|‡ØY?â0|/Væ?¹ŒÁ=3÷?â0|/Væ?ç]è‰#?¸yða?'ò?ÑD/éþíº?¸yða?'ò?êÿ¾ËPvX?¨o
hÞÉ?ÄÒ¾&¡?¨o
hÞÉ4FGL J0347.0-6400¿¤:£EIÀÀEÚà"'À;¼qáÄ«–À=_@©={Œ@?²õ`>Ú@D@¡±?ÔaÝÖ	Œq?ïpaêh@¥€éŸk@óĺÇ`¿ìolÕp«¿Üޝ"µ²¿¸®ƒ5ªø¿äVˀœ¿ì°<]ÔF"¿ïÿÕ"[ʁUNASNone?ܖґUý[?ҍH>Ÿ,?ᴖ·US?ҍH>Ÿ-?á,8eÚÇ?Õ©Áu¬$0?ݧ4KÔq?Õ©Áu¬$0?×4ř9
?À' ý˜ëÉ?äe3cyù?À' ý˜ëÉ?љ">¨?·":#"?ç35àý+ù?·":#"4FGL J0347.5+0722¿Ì¯ãGś­ÀA"åÞÊmÀ;oH-–;@À<šŒq'êS@!'µ~R?üÃ?ÕØå	?×ÈÛîBé?Ôò–'•¿@µŒ>gCÜ@½l‡'±¿ïþØþ^jD?ïÿñ‡—8–?ÙËëü<üá¿ËЎxSMÛ¿ÌØâ
ü˜¿ïû|b§,UNASNone?ïúK•¬«ž?Eus—ŠJ?FÑ©MQ‡î?Eus—ŠC?ïú»wúÑú?h†%–®?E ¸¸?h†%–«?ïžÎ('q?"¢ñÀ13-?ˆLuö#Ÿ±?"¢ñÀ13/?ï¯ÅՒ¢?vh$Ñûi?"Š›WxR?vh$Ñûi4FGL J0349.6+4026?Õ¢s	R™`À%GMƒAÀ:m@OÁßÀ<òö,A§@fdzÔ@ý¡Ä
†l?Ñ\^¥§ÄÖ?Öf.Þé}@;¹Ïš§@,ý ý{–?ã.žxük ?ïç¶}U[¿åçð¶6¿àH"íˆ.7¿ïÿøÞ£Žæ?ëóæ·YžUNASNone?ëË/ø­X?¼,åkeoÔ?ÀÓCÐJ¢?¼,åkeoÔ?êZOÚ©?Ì
uÜB,‰?ƗÆÀ—ñ^?Ì
uÜB,‰?ånñ(=d?¶­ÐD¸†‡?ÕÝ"¯…6?¶­ÐD¸†‡?êjÝìJǍ?±‰ÆÃ/»?ÆTˆNÔáË?±‰ÆÃ/»4FGL J0357.7-6808?è¯î(luçÀDO
å6PÀ;ÏrÎ\À<öòB9`@!Êy»WÚ]?ú6?Ýe¡E?ÖRÆ«ú?À£ÇšÞ¾?붖à+Ï<@J÷ñé'Ô?àq<þ¹?ïÚÚA)•û¿êòø°€eì?Ì®‰•Àq¿æ۝ }Ç?»ñÿPUNASNone?ïþ5PkÏ?-èþoðô
?.ªùC8?-èþoðôA?ïý•í4Ec?Pñ8â›<l?3P–]Ôçœ?Pñ8â›<l?ïªK·"í?‡d*Ûz•1?…mğ"?‡d*Ûz•0?ï÷Ø`øJ?FöêÔ␣?PO>k÷t?FöêÔ␳4FGL J0358.1+2850¿Äùy~…¬À2[YÿOÖØÀ:÷
"ù$À<\ZéZ¢
@°Áü9L@¿­½=Ñ?Õ¤Ùÿj+?ê7H €(.@.Z¡6F
?üÅÈkêó?íÝ	@¢C¿â›EÁ*WB¿â!'o°'¿ïÿýF\I?ïþÞݛ|¿ïÿý{ÁA~UNASNone?êɛ«ŠH?ÇFR`9?ÄٓýQÖå?ÇFR`9?è z°˜R?Ó¡»2‰?Ϧ=ž¼?Ó¡»2ˆ?ß](7ùÒ}?»†³b>%¯?àQkäÂ?»†³b>%¯?é®ò´Á?Å›Âý?ÉD5,û¯™?Å›Âý4FGL J0358.7-7403?è澿9¿åÀB£"ý*bªÀ;20:ZnáÀ<ˆ0bžZÉ@e[ç1@ÎàV?̒3ž½ð¼?¦òC~ÚÑr?Øm˵u˜3@fâ(~¤K?št.P}¿•²ù#hæ¿ç,—moo$¿â7¡Â]B¿æb§•¿ïí=±¼PUNASNone?ïöLYuÿ?Q_>5U"?SñgM%?Q_>5U?ïü\ÒÄPo?WI9ñþ"?=iÝ|Ž×?WI9ñþ"'?ïšM§*´ª?†î8‰Âð'?‰l–5RÕ¤?†î8‰Âðƒ?ïò`ÈÛú ?H
,ªsÔ?[>nH
¿?H
,ªsÜ4FGL J0359.3+3626¿ïá]%ázÀ)%òE,YûÀ:…¹ª±À<pÚ]¯@$)*Ü@ú'QT†?ÐtµÍ¬Ç?æÛÊ@«kÔ@êyþɟ?ö¼ß2ªø?ïmíCdٞ¿¹ÄÞýã|¿ç¼æ'æ¿îÛú'½˜¿ïû^°d?îtp–kUNASNone?çÀ`³ý/?ÏmÇێS?Ð>˜å¡?ÏmÇێS?Ôãà}¾¨Ô?Õi±Ã<`ú?åŽÁ «–?Õi±Ã<`ú?ؽòßÒp‡?·"Pœg?㡐Ǽ?·"Pœg?³mÓ&C¬?¥›ºd/â^?í'Eœ»7Š?¥›ºd/â^4FGL J0403.3+1249¿ì	7Ý|R'À<¬€"ÞÀ:èù@ÉìÀ<'ä™r,@VŒè±.â@?)á{?ÀӚÇA«¿¶ QY9S?ö̯UÀô?ú®ä­³,?ì0©€—j¿ê;÷'X	¿ÞH¿nÀR¿éÐ"¢lQ¿ÑvÒîL#¿Úé<+)UNASNone?ïéB…«[¡?hj˜ûØù!?f½zT¤^Ï?hj˜ûØù?ï˽z=m'?'cM<ç?z!BáI7R?'cM<ç?ïcÍt¯â9?«tcÌÃá?"†Qj¸Ý?«tcÌÃâ?ïOÕz
^?‡D†ôÈ¡F?–P¿T?‡D†ôÈ¡F4FGL J0405.4-6929?íþÍV'á ÀC©= ò¾ÏÀ:'3æÊÀ<q´üÌnÙ@*£ÉO•@mt­P0?»‹/ÉqM ¿˜ßÌȉàÙ?ݺÛGŽŠ@	‹QC>™?ëwA 3fµ¿ædaX"¿éË¢«;-¿Û£J<º™¿í°¥)œ±¿ïÿÿ&¦³UNASNone?ïþ¹íýª?*DLl{'?.a %V'?*DLl{w?ïýÉüœ"?L.Ò=Ò&_?1·XáX?L.Ò=Ò&^?ï虡.jP?lO¸ˆ|‹?gf^ѕ¯¼?lO¸ˆ|€?ï÷CH	¿F?AUê­ôŠ?QyoìuV?AUê­ôš4FGL J0405.9+3041c¿À‰j-k±KÀ/±_$RÅ À:Å><À<
Bð?˜œ@Þg~ê@%
ÌÜ­?Å["J§îò?‡¾%·l	á?Ãî;ÝPÔ@¬G±"?îß"o–Ñ?ï´÷ù¡A.¿ëqM_¯=¿å8׊•ñ¿áýK 'ß¿ØœbÁì!UNASNone ?ï"ò¢•$?'óf‡çö"?‹WZ¶øc?'óf‡çö"?ïÝÐk˜î?‰È,äDy?qxÊ3‰?‰È,äDx?îǒþÀ̤?–ý¦›|™?£†Ðó5Ç?–ý¦›|˜?ú§ô?}f'×^fç?Ž{AV;?}f'×^fè4FGL J0406.2+0639¿ç—oRÛÀ@Ô^'…ÏÀ:£Àd¾À;ÿt²G@{Â4moð@l¬#	"?ÓYùñs¿'ѯà'â?ÐDƒEW@ž0ªlЎ¿ÍÑð£Ä7¿ê1[Xo®¿ëñ±¾SF¿Þ—\R'G¿âŒœÆtÃ÷¿Û|c=gµUNASNone?ïó.%ó?Wàþ9D?Y£µðÏË?Wàþ9D?ïþ#éΘ?Mù¶ýÇ©Y?.ÝÁcq?Mù¶ýÇ©X?ï¼Ð.oÒ?€òf\s7?€øKôdX?€òf\s5?ïù4µçw?;õTbjÖ?K-(b#å?;õTbj¦4FGL J0407.7-5702¿ç*`oKø'ÀF4¯O
"MÀ;/øIRYiÀ<ºª¤ƒØg@'šúlÃ"@Ù{f¨«…?¾/p[áÇ¿¹‹ä$WM?ûúÃ.¾Y@[ŠPÑSÅ?í=™Þ¸Ý'¿åÉ>ÃNŸ¿æ:V=#vþ¿èw²ß:みæ­ Ε?¡>S‰ÈUNASNone?ïð}\àú?\иñÍ°:?_ÅF>Ú?\иñÍ°??ïÙk©Õ
!?‰:i)Ü·?sJ+zïN?‰:i)ܸ?ïQŠ_ØÚ?FáÒ×¥?•Þn´äº?FáÒפ?ïÃDj"v®?m?d®È?~]ʽĩ?m?d®Ê4FGL J0409.2+2542?íõ½BÀ2à}=B€®À:ÁZˆâ'1À<T3\MÞ°@ x×­{xÇ@#!m8?ƈï-ö?°'ö¸»F?ì2C¬ýú@7;«|Æ?ïï"'`í׿çä‡v¿Ôƒá6]E¿ÓØ-=¥Òã¿æ´Ã { Š¿àPÂFbUNASNone?ïý9IK²?2Y·\í¬2?65µ¢oì…?2Y·\í¬$?ïùGC¬Æu?g3:¤À3å?JâñLæ-»?g3:¤À3ä?ïñ¿yc¦ ?k4	Ã4\?\
8²Àé?k4	Ã4X?ï¶Gç~¬þ?m*zØÍn?'n TÀI?m*zØÍn4FGL J0409.4-3822¿çÚ½/ù7ÀG´éNã'âÀ;
Vƶ2WÀ<D@¡±@ ©"- Ê{?ú~e`¬é?Ó듡ÝàÆ?ÜÈ?xæò@*Ï1+7@ŸPW±A׿å P!Öi"¿î؞ý†¨ü¿°‰%BûR¿ÇìÎ_tÞ¿åg쮤"¿å%Ü2›UNASNone?ïéþb»?b-j<þ€;?füDãN?b-j<þ€5?ïò'¢\ï7?u'·ÕTY?ZÜ»F!9?u'·ÕTX?ïNÒ¤Äê‰?'ˆ‹Ö""Ì?–%«gb®Ó?'ˆ‹Ö""Ì?ï^ÝO½V¨?"k±O_z?"$VU*ê?"k±O_{4FGL J0409.7+4006c¿Õ¡,ÃòftÀ úG²À:'OÐ"À;¦y3Ȅ@ô¾}ÿŠ9@)YE³Æ?Ór½â¤$?滄Üޓ@µŠáoò@02…8cŸ?ïìv`Y‡?¢Â{÷-…¿èòF+]|¿î3¡˜@©¿ïü´%t¿ï¯žŒØÁUNASNone ?㔷i"+å?Ð<§ôíˆ?Ø֑,ר5?Ð<§ôíˆ?ÆùÓÇP?ÊsÓò1ñ?êA‹9 -?ÊsÓò1ñ?Ôô6`ƒa½?ºÒ-ð0šÓ?å…äϾO!?ºÒ-ð0šÒ?¤PÑ|.£+?Š%'"¡ž?îºòè=Í?Š%'"¡4FGL J0412.5+6519c¿ê".—Õ+@$c€ÞôÀ:÷e&ËFÀ;ˆ`¾†¸ì@u3Ú¢ù?@±z`ï.?ÕJ*7!?ì~kàùª{@	ÃJ¢»K?ül¶-‡£?ïô´<³¶¿ÑÀa"V¿ìœU•:¿éEV¶ÅúK¿ÞgÜó‹}w¿ðUNASNone ?àDUÆ?ҍ¢	?ßw÷×Uöt?ҍ¢	?ÑÌ~8O÷Å?ÑidÒ*´%?çÀãØ?ÑidÒ*´%?݁ïÊæùþ?·±§'¼Z?á?Œƒ?·±§'¼Z?±Pýœ÷¨®?¬«—Óáý?íÕàLa
ê?¬«—Óáý4FGL J0413.1-0304?èÃùP[…ÀB'žùTëÀ:7]à…ç5À<$'sZj°@‹¾‹–v¤@óæfÑÆ?À·©°=?–"ÆÜüMw?Ò¨~oǎ@8™E5ê?ïê
*%mx¿áçKh´€¿ãåþAcøx¿êkGa=‡ ¿ëQƜ1$¿ïÚúWI'ñUNASNone?ïÏ«xñ[ß?|	{-YY
?x*C‡R?|	{-YY
?ïܦ%`u?ˆø÷Þ;›?q¬ítÏÅ«?ˆø÷Þ;›?îÛ³&ݾ?–À¸¹»ä?¢D͞'$?–À¸¹»ã?ï"aq—¹_?w#hϪ•õ?Šç£š¨?w#hϪ•õ4FGL J0413.4-8609¿ÞÃٔúÄÀ=ˆ]…TÖÀ:ԄÁ›@cÀ<yþ+êi–@U£žU@?ý«>݋a?ԉ¢Á
¡Å?äϺRvÅY@‹ðÜvü@m÷[ÐL?ïüWÔÓ+Œ¿ÉG ½û"Ì¿ÝôÝ5¿è£˜ Õú¿ëJ9ßö¿ïøŸ^›—UNASNone?ïñY×,?¥ i–c?ÜÔÅŒ?¥ i–c ?ï0¨îVU?¢Œ­¥èÿ¾?Œ³ÕÄjjÛ?¢Œ­¥èÿ¾?띬iPž?ª–uê""û?ñ‰NZ½?ª–uê""û?ìì¾wÑö?¡v°SGn4?¸šAwÐK?¡v°SGn44FGL J0414.3+4522?ÝÈ
õ¦ÀVn¡žJÙÀ:ð Â'ÆïÀ<4؇3@!I&uà'?ÿëÕ:Y˜?ÈB4‰´t?:9$A†? HŠ]f@'ݳ$A¿ïþ؝»gJ?Ýy¤{õľ?ïßd™¿æÒ®Žd•¿ß^Ù¿¤p7¿äq`Ëò¥UNASNone?ïù[ƕ?P¦b[âþ?K¶åª¨?P¦b[âý?ïú<aåÒº?O¿~þ€f?GxhµH?O¿~þ€g?ïªçTî?'Öw0!?…F=*ÄZ?'Öw0!
?ïÝ&'XÞ?dÎ|[.?ql·Söu?dÎ|[.4FGL J0414.6+5711¿ïgà‰!ø@͖ hÀ:nìzçý«À<!¬%XC@ á "_Ps?ÿN-E	?ÇoØ‡Àÿ?¹ÝtÉâ?óîZ¼8¨@gք±€?ï¥]S˜.¿Þ#uP5¿ß¥I»ŠÛ¿Ü("Œ,ô¿Ølª'õé&¿êkó™mûUNASNone?ïú‰×ß?B û€˜î?Eء˔ƒñ?B û€˜ñ?ïó8†è¶b?|€ëÅmî?YŽò."<=?|€ëÅmì?ïۗÅ&Î`?x˜\r]¯?r4l˜Ð?x˜\r]¯?ï C!¥þ–?sþjûÞCD?‡ï7–€ZÌ?sþjûÞCD4FGL J0414.7-4300¿î¸AâdjÀGVìÔªÀ:Ô qúïÀ=Û4nœ–@ÿ
Nãgï@Ü¡Ü^:H?ÆÒv‰Ê?"a(å@I0¾
í)?÷I6W™ƒh¢"K§¿ ¨áž)¿Ýýj#ŠHÄ¿ì"PŸTÄ}¿ïþ‰]aZ
¿îÌhÞæªÄUNASNone?"VQ,ñ3½?³q†5ú¦?ï]Mv˜vb?³q†5ú¦?˜þ-ãÔåL?¯Y«X'ƒÉ?ï8áXÕ?¯Y«X'ƒÊ?´ìSŽf?£uR
»c?íbnŽ3?£uR
»d?HVÍՍÆÄ?7"ª4?ïùêLŠœ?7"ª4ž4FGL J0418.4-4342¿éb>K™«cÀF¿á2µ^òÀ;ÑÅ6ÖUãÀ<îì$·o@"-¡À»¡?ödc§oE2?áw¿ßÔft?ɼŸV?ë~X€I¼b@¹@œÓ4ñ?äÎô?¿ïÿêÁf½?ïûÞ.ôà¿àòF¿2/¿ï1½è-{c?î2þ…°UNASNone?ïöAÓ¹]?Vsî?S|XŒýE?VsîŠ?ïý #wÐ?PáÀe?2ÿäA{z?PáÀe†?îIJŒi?—Å¬ÌÓ?£¿×9nÝ?—Å¬ÌÓ
?ïô€ ì>Ñ?V…âN†½Ô?Vþ¾''_î?V…âN†½Ó4FGL J0418.9+6636¿ï ZSDÌ@'¬%XÀ9kÃA2Ð7À<
òPŠ@Q˜âdŽ ?þg:×lc?ºØ6bg©?ظ¤¡µqç@!ŸØ­«ŸV?ûò§b,
?ïÿ`Úá8¿Íù/Lñ ¿Ô9-H7§¿áß¡@,¿íz4y"P\¿ðUNASNone3FGL J0419.1+6636?Šögui`˜?¢î¡mù¡?ï"&b*Z}?¢î¡mù¡?rQœ×Íj?¯a"ë?ïÛ\ÆPe,?¯a"ë?"ñeR¨H"?ŽIwXlžZ?ïXtÕj½¾?ŽIwXlž[?GsôGX?9=£g?ïú#ú®??9=£g4FGL J0423.0-0943¿ïþòл?¤ÀB¨'_ét£À:ûPÍwíwÀ<¿:4¯46@h÷9±?ÿþó…õ?Í\i¢Ûâ"?Þït—'e@ŸÜœM©@ˆë؀µ?è-'	'`?»`̞¿Õº˜b¬¿âuÛ³¿íZ·qõO¿ïùì?®ÁŸUNASNone?ãò¯ŽõM?ÈûƒW"‰	?Øô âf?ÈûƒW"‰	?èP4Á$q?Ѿ&»4Š?ο-Èûn=?Ѿ&»4Š?ÑÍï]—ª?¸ÁéÒG?ç~Ñ4+?¸ÁéÒH?è'8ûn?°$‹3w=w?Ï·­·K?°$‹3w=w4FGL J0426.5+5434?ïã®v
áí@ûH
[À8VĘJåÀ;(&Ú@èÛ2k71@"÷Ãñ[ø?­€4¡Oùñ?Ùô/|ÅM}@$ãBؤ@ÿ:)Â?ÉÍ8¤û¿×ÄaÄ@6Q¿çÍù½ÆŸŒ¿í¦Á Hà¿ïü¨'Zà÷¿ì´¿ÍhUNASNone3FGL J0426.7+5437?"Jéì ?¡NŽkª›?ïe¨°ŸBÿ?¡NŽkª›?ðZç¬*?¡"Q@!ë?ïÀïJ0¨?¡"Q@!ë?ÇM|÷2%?¶t›±ƒ&?ê, Â3v¿?¶t›±ƒ&?ºWi5އ?Í7wÊՙ?ïÿ-D¶R?Í7wÊՙ4FGL J0427.3+0504?ו5U&åÀ<ÁR*o?SÀ9hŒs@À;¹ðŠA7@X'ßB@°†£Ð?×9''¦¹?Ã'ǁ&?þ*9ªE¹H@
j»q/ÿÅ
x¹z4¤¿æia#pÈ¿éÆ3k	¿í\¡V&}B¿ïÿ2 ;IW?çZòʍWlUNASNone3FGL J0426.6+0459?ïýo´Ù'?8í´Šc¡"?4'Y3w¸‹?8í´Šc¡/?ïû/W«kb?`ÈeC¿Ë?CB¡RRxŠ?`ÈeC¿Ë?ï)i90ëÝ?'89£F?šÒØÙâ"O?'89£F
?ïêŽvc›Ä?WäQÝƜ?eq‰œd=?WäQÝƘ4FGL J0427.4+6433c?äêï¯@%'"ÂqÿøÀ:.®ZZÀ;¾@=ñŒ@ìýåžÝ@[yJ]?μ~`ƒ"Š?ÓÄ\:é`@nò[Ҏ®@_îZ;4ß?îA²¢i¿…¨ÛD\7¿çžÖà!t¿ïaMl·ä?«Ò¨²FÓ¿ïÿŒ!áÒUNASNone(?ì~¬ùÆmÒ?ÀªB ‰?¼
˜1̑s?ÀªB ‰?ë"0Qt?Ë?*0
?Ãwç>º/Ô?Ë?*0
?⽿ÊOÚ?¼I#íP_?Û҄€k`L?¼I#íP_?ícx~áÛ?¨ªìü²1½?´ä<ñ'×?¨ªìü²1½4FGL J0427.9+3632c?ç²séBoYÀ û`'ŸÀ9'É"\h·À;mθ_W@­ÔI@²U'þ?ȾfØ|-x?×pZ›ü@‡è|U»ô@q1¼'?ïÛʖ'¿Ü‹}At>–¿és"ý}™´¿è‰ŠøìæH¿ïèí"Ãq¿ïé¿KÚÉæUNASNone ?ׇ¶''Iº?ˇF—þ}?ä<$·7[$?ˇF—þ}?Ó6KUƒ?Ï ß®Å0ˆ?ædö·ÚU=?Ï ß®Å0ˆ?ÛhŠÕˆ#?¶úðØ6°æ?âK¹:•;ï?¶úðØ6°æ?Ð2ÕwSt×?¬äëÍnã?çæ•DVE"?¬äëÍnã4FGL J0433.0+1327?ãùÙª"kÀ6©¦
EbáÀ;8×ôH;ÙÀ<튯@ÎpþDéê?ÿÞ5Ìj§?ÓiÎEêœ?ïÿwåëo@Ìã=Qš'@@¤‹¿êÒ2g[Y¿ïénù²Þå?ï½è=–Žw¿×Àó°fe¿ïÌ&´Ÿ¯]¿ïïNÒöUNASNone?ߎØ<±ß?ÎÆ«××q]?à8"áð§?ÎÆ«××q]?Ú\ó<D³?×@%½`¦?âцxáݦ?×@%½`¦?×ö6a``#?µ§Þ²Áôà?ääÏOÏï?µ§Þ²Áôà?Ò ªôx ?À8æeµna?æ¯ðª…ñ?À8æeµna4FGL J0435.5+3232?²Ù-0rÕ"À$
ƒ{á"À:ºÁ濽À<P[¡çEõ@.v‡›À:?þÑטةz?̍ø%ÁÃ?ØèÒý='í@	ñ9þÿO@õõ•måâ?ìÀäbÈ?íúVrÓ\3¿'Š FJÖؿމlLþ¿êz:Ä!, ¿ï"ž"?pUNASNone?äW9´4ÿ?É8aÈg?×QŒ—–Ô?É8aÈh?ã4s¥¦™?Ó¶ˆ<y?Ùá—´²Î?Ó¶ˆ<y?ãße"=¤?¹Ä™_½T¾?ØA4÷…¹?¹Ä™_½T¾?ßÂå}:nþ?·v› ˆx?àAbȁ?·v› ˆx4FGL J0436.9+2915?ԖY@ñNÀ'äAVâdåÀ9ÐϟåãõÀ;wˆ4íG—@3·EQö@Œ²`9ü{?ÁçZS<=?ÎbZû¤&@ú¹o!÷?ðŒ+$U?Öº'#'à¿à·n=h¿ã|¨Ý"U¿áüî
ö¿îLb-<¤¿Ø1Æáü3îUNASNone?»L"‡5#x?¸ß•`:?ì–mo['?¸ß•`:?×É­ëËÏ?Ô×T'i˜n?ä)
rš?Ô×T'i˜n?Ñ»ëeÇê?¶ìïõ\€?ç"
M|œ
?¶ìïõ\€?³!§ý6û?"°¯Q›'?í›Ë Y!?"°¯Q›'4FGL J0438.0-7329¿ïŸ
VíHÀA—ŠC»@³À:n¢‰,dÀ<}ƒêXÏ@ ¦'æQ?üADˆÆ¿?ÁÅøâG]?´P°Çˆ•:?ó°¹÷2ú@¤h$V¡w¿Ü½ò%Kê¿ìI‰¡Sø%?¢GŸë‡¿ÙàP7Oøf¿ß\*Ãx[¿ßd3›¸Ø¤UNASNone3FGL J0437.7-7330?ïþ‰eU×ð? pÙÿ¹N?'iª¢\? pÙÿ¹n?ïýàˆ9ژ?Lþ‹Szh?0û¾1+Fó?Lþ‹Szb?ïõ+"™ÀÛ?f¬O™ûö?U¨ØÌ~K+?f¬O™ûû?ïëÄy¦ÀB?R}`Þ#Ñç?d;†Y?¾A?R}`Þ#Ñï4FGL J0438.2-4243¿ä#äÖNÀDø¿p]À:¾Ú`3FÀ<Lð\@D&äpX@g ã¥Vf?Á"žy_g¿®	§ô{<Œ?í®"áÉ´@¸"ŒòÂ*?äYo<νh¿ê$DîFš¿æM™{f¨¬¿ê—v©ªˆÕ?γŠ›úÇÝ¿ïÿæ4|ßOUNASNone?ïòé½~ã?\oMkø[È?Z-؅9…?\oMkø[Ç?ïý£QjwL?Põ":›¶?2åt¬E¤¶?Põ":›º?ï"þ)Ñaû?‰¨x ®6?ŽÀu‹§b?‰¨x ®6?ï÷æÚ,q?F²ìÎSØ?P2K§ç¿?F²ìÎSØ4FGL J0439.6-8322?Ù²ó¥²|-À>•Ëeè'À;%Y>_· À<€RnM@"wïвà@ˆ:Ùð¡¾?Ó?Õ"[ʁ?ÇĕEÌé?ñ(º3m?üNøñ˜ß
?ï÷¿¾€^då¿ãY8œ(À¿âV•Ù¸é¿ï]]ÿ¾¿Ù>Ÿ¿ÎbUNASNone?ï½6ó1j"?·}ÅO¶Í?€²C3¥_
?·}ÅO¶Î?ï~…W'Òÿ?Ÿ°«!$?/U
¥ $?Ÿ°«!#?íïu½sò/?žärÔÎ$'?°"R`n€?žärÔÎ$ƒ?îÿˆ®U?•‰–ªü?¯®°u ?•‰–ªü4FGL J0442.0-5432?áG5²o&ÀD/§íåÀ:¸8!ïÀ<¨»5˓è@/ëï|Ð
@g­"ãY×?¼ï"ãñ¿­ëþì.¼×?ð:µ´)@v•]ŸÃT?åsú~
òͿ唐æl±¿çÝB 8š¿ç¶Šþøï¿ïÿpޏlð?ïýÕM¤ÎUNASNone?ïø¼¿X?Oì-±ÈmY?MѪ¡m?Oì-±ÈmX?ïÚC)3ÔM?…×"Û»_ä?rÞkfÙ,?…×"Û»_ã?ï»í#]¹¥?€RëÒ?·('–±?€RëÒ?ïÖ¬ƒŸÇ?gÉEeôaÊ?t÷)¾0¶?gÉEeôaÊ4FGL J0442.8+3609¿ïÔ{uÚÉÀ¤¡4˜ŽÀ9×äQMÐmÀ;ƒÔA5Tv@QBŸ@f1rhÓ(?ÆjEî÷š?Ño§BN¯@*F"bH@ªÆ>¾,¿ÉEø\Ȃæ¿ãß¤¬ó¿è€fAÓ_
¿í¤]­Z@¾¿çIžÚv.¿ïì‡b_p©UNASNone?êg'"A¥?Âtsê±?Æaõ²ûÝn?Âtsê±?褝ÕR?ÐhI(è8z?Ïåmˆª·°?ÐhI(è8z?â'nÆËÙ-?¹9¾3@¦?ÚtìrhM§?¹9¾3@¦?ãçÞRpEÉ?·ðl´í 6?Ø0C[tq?·ðl´í 54FGL J0444.8-3514?Ô ×œöãéÀDçÝÊKÀ;k%ÈçdÿÀ<Ëå+hc—@sÆxIè¬@®'r—Í?Ð!DÚ$¤?°g3BE?Ü´_c@ý'öÛ?ïÞ43
s†¿ÙæFñV¿å"ÈA!ÞL¿ïýàÀõ~?ïàŸ°4¿ïñ$ЙàçUNASNone?ïÿxñÐí?:³HÆ?áÅâNf!?:³HÆ?ïþw^vÜÔ?F¤4|ñ¡?(Š'2¿ú?F¤4|ñœ?ï…ãêÚþ7?ˆ±3s‹•?Ž‡I@rN?ˆ±3s‹"?ïÿa¡¨£Ã?µÝ"¹Ûv?ËÊ뇽}?µÝ"¹Ûü4FGL J0445.7+1535?à[´ó­	À2ìUC(s½À:FE­‰:§À;·áñ÷ÿ€@ĆØ!@Yx"væ?Ó0p ¦ÿ?ÜBéŸ"w@	˅¤ð@ÐrùòŸÅ?Ѭ9d$­¿áËF¿Ä§¿èO¬½ã¿ï~µè"¹¿ïºú<q V¿è…™!y¢XUNASNone?íD!^îå0?¸õè¤	‰?µÞõˆÖƒ?¸õè¤	‰?åÁ–{@Q~?ÑIùUwü?Ô|Ó	]?ÑIùUwü?ã«s¼™ÛV?µÕ GWãÐ?Ø©†ÌIV?µÕ GWãÐ?à}Xnrï¶?³ÅڊõÁ¿?ßO# "?³ÅڊõÁ¿4FGL J0447.2+2446?ïÿ:©<UàÀ*]ÌcñAÀ:–8¦ÿ´À<LB‡ö@vWNñTÁ@æYeÌãs?Ò‹eNce?îÕëY€@~¿ù³?üµíbC—?ÙqÒàãG?ïÂQHÇïî¿ÐÕao0º¿êÕTáä·¿ïÿw¯d:?ïñ™À…ì"UNASNone?²j"V~Á?ÀÜ¥)[v?í²¯u>)?ÀÜ¥)[v?¸Y¤­ G?Åïý7®2r?ìôÞ+jKø?Åïý7®2r?Â2èžÑ5?ªÇÙñ틦?ë~sEØK²?ªÇÙñ틦?…\#݅"˜?x' ^lw?摒p‰éî?x' ^lw4FGL J0448.3+2743¿ãÌÛ°À&TŸ"…^À:³jû÷]À;«Lg·Ÿ>@]EÌ=î@U8áÈÝT?Ï'öüK@?ҝû¾|Òä@*à~Zy@¿"Ë(²Ò?î–éP'¿Â"ž'¨'¿æ[™ï)îç¿êB­#º¿ìùYó'\´¿ïõø	'y:UNASNone?â|ì1ÃÌN?É2±Wù?Û'œxgc?É2±Wù?èørº¾=à?ÊÍ͌Fí³?Ì5?ÊÍ͌Fí³?á/W°ó?·±Ù¶o<?Ý¡éQܞ?·±Ù¶o<?ãÇDÀ&‹ò?²"Luþ
þ?Øqv²è?²"Luþ
þ4FGL J0448.7-2116?êÓ»-ýEÀB€ýÁaÀ:wSeØ¡íÀ<láçDò@^¢›öÁ@‹Âßä?Å,ËåòÍ?Áǎ^ýçL?÷ÈÙm²‹@Y>:"e±?ï¢1þªÀ]¿â«¼|±¿è¢R_ô1k¿ãinX£/E¿ï½vþ«¿ïð­aÍzrUNASNone3FGL J0447.8-2119?ï÷ä6J1?Q'‰ApÞ?P7"kអ?Q'‰ApØ?ïþJoéˆ?J÷¯AŒä?/ËYgp$?J÷¯AŒä?ïÜ(m7/b?rnáÝ"©?qëÉdhNÑ?rnáÝ"©?ïö__©žå?B7ÓZÄ<?SA@¬Â4Þ?B7ÓZÄ%4FGL J0453.3+2843¿åd_•UÇÀ#
çöô¾ƒÀ:3á @è(À;¿p¨È@ÅXQzÆñ@%ن³U?ÈVãçp'?Ñ®äïÙAO@»Ò#Mââ@ðßP²ö¿Ñ=˜|c'î¿à£'÷Ó¿ämä£P¿éæg"N¢¿è4©TøÙ¿ïøT<jUNASNone?ïÔ…¤¬ã?Bk•Y*?ŒŠÞ–ÔÇ7?Bk•Y*?ïðKFÏ?'0éâ¶?_isÉöc…?'0éâ¶?ëÙi(™R?§5lfóCè?Àš[_…šµ?§5lfóCè?ï}»Ðå/u?y®ƒdÓì??H…ãZe?y®ƒdÓìA4FGL J0455.9+6757¿º¦¼Èë#@.NޗÐk¾À:ô§vÑîuÀ<·ö:"`L@ ‡y{ Ô?ù¦,ƒì‰?Ó#½¿"©@?à¸æÁ?¥Ý@€':O‡'?÷ۑنĀ?ïè;B¡:M¿íÊJ µ'-?³Ó6sXg¿ÓÏF0Š¿éBas7…¿ß?|žJ®UNASNone?ﻯ"W?š…ær>–?;ê;y?š…ær>–?ç°¤Xz:?ÑR*­tõ?О·Oç‹?ÑR*­tõ?íГ™¤?¡b5߄?±{d{2á?¡b5߄?ã*	y‹"?·(Ë¡ž}?ÙÝ«íèÙ?·(Ë¡ž}4FGL J0459.7-5413¿Ïn+
¾ÀÀBíZ[–(ÌÀ;Vµ–Ob>À<è،ôo©@û¾Ù6?þˆw'î\j?ÛCú*Óé!?¯9X';§ ?Ðú`ƒÎV?ùêmÿâÎÂ?ídÈÁû7™¿î;.¿±q¿™]©&¾8¿ËéÙøÚG¿á#[NÛ/f¿ïÿ%ålÖÃUNASNone?ïÿ¯™LÕ?ý›½@?JÖeH!?ý›½0?ïùrÂÀJÃ?jCkßZ¥]?J4ôþÔ÷+?jCkßZ¥[?ïÜ£†#—ð?yƒ¶'·Ì?q®<î4b?yƒ¶'·Ë?ïÜù5A‡?_Ê–?qƒ}å_=?_Ê–4FGL J0500.9-6945e¿ÅšH~#0ÀAeÕQ֌À8¨7æ÷~À;v8è†@~ÕØd/ª@Óo1?¦+±^²<ÿ?REbåÇRa?³WÔþ©c@=`4H1?ïçë ÊÐÉ¿Þ[]‰H¾¿ã»üР–ä¿àô÷Ãñ[ø¿áF]v'Ï¿àïኟUNASNone3FGL J0456.2-6924LMC-FarWest?ïÎÓ=}¸´?rÙOÓø
?x–aA#¥¢?rÙOÓø
?ïöH:§x?wÍ2ãš?So‹ò±i?wÍ2ã—?îŠ~ÓE>s? .5ù
u?§XˬÌ? .5ù
v?ﭗ"g)ç?ssæ‡Lzñ?"š7f5†8?ssæ‡Lzï4FGL J0502.2+3016¿ærüõÁÀ+
€òçÀ;)ÿ­Ê©À<7b• Ž@ Æì)Œì?ùِʽþÔ?Ù¢‰bñO?Úìåq?ûmªx.—@,XÛäAÞ?ïÿùëñ¿ïýÅB"Ð?ï}[À›<¿Öèf»ö»´¿Ô©n)©¿ïý'€›pßUNASNone?ïý|ÖÅ÷?9ªÚ˜0G?4I×`L¥?9ªÚ˜0G?ïü^ÑQiù?btî^FÁ?=	ut°8?btî^FÇ?ï]hûI[¹?;‡(•+k?"Rà–ÔˆÅ?;‡(•+l?ïʏeMú€?q¦ÄkҚ?z¸MYÀ%?q¦ÄkҚ4FGL J0503.8-7508¿Ôò8r!À@ztBÇû­À;U­…ߨrÀ<¤¬Okx@ÆWÄb&@z…ص?ԏ&#*Q?Ï1¾{{?ñ'ºÄŒŒk@_[]ˆ¿ïù "_Ì?ïúŒž3‡A¿ãb°Ï@E¿å¡"ßþع¿å"PŸTÄ}¿ÚEÙ]ÔÇmUNASNone?ïßeoû?iøÃn?pwqÍH\?iøÃn
?ïçڕLŽu?"x¿wmÚ?h%j³q‹"?"x¿wmÚ?î$ÃDô—?ž­sé¹?­³Ë¾¶ ?ž­sé»?ÒVb­?x· Ý@•?‹ÛKjgT¦?x· Ý@•4FGL J0506.3-0620c?âWŸ¨«Á_À:6ŠçO/À:¦IÚ>¥WÀ<O%üéË
@©{%2h@š±ý=­à?ËnŸšåt?¸d ,?éžu "se@JÖßuEý¿åEv+ÖG ¿æ0©€—j¿âhx>Õþ¥¿æTÑ]Ö¿ë®IW¿ïûÍÖ¸UNASNone ?ïèŠs	‹?g¢ƒœõ}?gãuŒötA?g¢ƒœõ}?ïé'«œ?…ÿArŸ9"?f=mäTdw?…ÿArŸ9"?ïZM/ié?Ž5ëê¿ æ?"¶ZÂß#?Ž5ëê¿ â?﹛bê5}?máÜÈޟ¯?™'Er Ò?máÜÈޟ¯4FGL J0506.6-4629?â6¨CÀB{<`ŸÀ;v?""ÆÀ<Ó§<ð@!>÷þSØo?ù(¢› ÚÖ?ÒQ>a¸«?ËkÄIE™<?þ5ctCž»@-œsÇ-¿îm"wú¡?蔩ÀXJD?ïHã—­¿Ý ~Dÿcx¿ÐYGŸœ¾¿ç"…U>÷UNASNone?ïø–°Ö%?N•Ü·n«?M¥<§kžö?N•Ü·n©?ïý—D)8Ï?RœàkÐØ<?3EÞ¶9‡è?RœàkÐØ:?ïº+¾wÿR?€iã!ÒÒÏ?ub+ƒ?€iã!ÒÒÐ?ïï¬ñr?SS"ƒe
1?`øSôB?SS"ƒe
64FGL J0506.6+4545¿£5ç«ï¨@

Ý8TÛÀ;@{¶YÃÁÀ<r%ÿn	É@"‰ioZUâ?ûŽnD—à?Ö§;®+÷Ö?Õ¥±ÀVò«?òésçXiN@ïÑ—Êâ¿ïÐaò¹F?íÈúz…\¿ð?ïÿþBe«+¿Ó`dYEìs¿ïþpéw'UNASNone?ïæqÁÃòu?oTfÇ"?iŽ><
Šò?oTfLJ?ï2ªÛ8Yf?·dV>J2?™ª¤˜ôÓ?·dV>J1?ïQ…¡53?ŽÝÚý†Þ?•ÏKÝYY¢?ŽÝÚý†ß?ïÁÜ0Ž ?{D4ÂÃ$?ç¸ïô?{D4ÂÃ$4FGL J0512.3+3329¿ëÚaÔ±œ®ÀLF__áèÀ:v9´V´BÀ;üz,€@ ŠŸb0?ú–=Ć­.?Ó¥àú¬.?ÜÖÈäŠÙ@æÎãþAº@0@0Fĵ¿áÒ)˜¾&¿ð?ð¿Þ¨'¤W¸¤¿å>8ŸÙ¤¢¿ïúúý·¦JUNASNone?ï˜Éîá<?Œ©CË$¸?‰Í¼DG°¹?Œ©CË$¸?ïðŽw+?•+iqùOF?^ã©ß?•+iqùOF?ë
…È7§á?¯¥¥Ҁ?ÃÕèß!`y?¯¥¥Ò?ï?¦ÇÓ#?ˆF:i8?˜'E›¤?ˆF:i84FGL J0512.5-2201¿ìíüÕIÕ¡À?êÈ`V'À;&k&¿‡jÀ<~ž43
@‡k;p|@R ÿT–?Àv_'Çp¿¾,8Ã
@³"ý*bª?ú–ÆXêR?ï÷%  ¿åø'Už˜¿ëÝLâ0â ¿ÞµíãðQ¿ìn<ô}ÿ?é¢ áÌäUNASNone?ïǑ/Nì?}µ¦f…´O?|7hXòŠœ?}µ¦f…´P?îããÑ-Ã?µýÊS·ÁÒ?¡Î!Âí#ß?µýÊS·ÁÒ?îöHÅþeß?"z',¢üe? ›s ¢?"z',¢üd?îžÈR|¥Ñ?˜ËidÞxA?¦zØ5¢ü?˜ËidÞxA4FGL J0524.7-8304?ï3ÁåJˆÀ=~¢‹°£À:Mó™À0À<Tˆ'@>Ãز^7@ˆ$&Oö?ÍÛ·`Ô×?Óù|ƒ3Pº@ÿÞr¿?ü÷f³›x¿àHksì`ç?íÁú@£^>¿àJÞ˜–¿ë;›í0ðc¿ÚED"ٖ¿ï÷3rôcUNASNone?çÑû¯Uóf?ÉĄïiõ?Ð\¡T5?ÉĄïiô?í2á¢ËT?ÁòØÕ©h?·^hòé¥^?ÁòØÕ©h?å'3$!?¶¥\hUB
?Ôû󙷽Í?¶¥\hUB
?æ!ԃíW?·Ö[lm_Ä?ÓÙ¼Vø%T?·Ö[lm_Ä4FGL J0527.1+1152¿é¶sdëdÀ)[	¦qï1À9Ó@ŽeˆñÀ;¡¹ìxk@Ì´äxºý@‹®9cÎÜ?ÇV†
JÁ?ÈB¡û'Ýé@-©¼&Œ\@*ø==ù¿ÏZ¡¡¥×•¿ç¨^žEû¸¿çâJãS!¿ék8'ŽºC¿ì.4@ylÓ¿ïÿPþU0UNASNone?ì´$ԜÅ1?·n¯#‡{¶?º^Ù[Öx?·n¯#‡{¶?D̲=?·èIðM?§U+³4Ü6?·èIðM?èÖ̂›w¹?µ6º0¥L?̤Íõ'!?µ6º0¥K?íks:›Œ&?›Ž*§?4Ü?´¤f+#žÐ?›Ž*§?4Ü4FGL J0527.4+6647?à
ý!ýç'@1=¼#1]À:ÄÑ2À<¡S¢>"@›_-b
ç@ŸÅoá9?Ãaó$¥PÝ?¯fÿ0ø?ì(›?6 Î?ù÷Xÿ ‰£?ãÞDno¿à_0?ÿä	äO QD¿ßÆæ#5U¿ß¹"@"DÆ¿éÇaS/UNASNone3FGL J0527.3+6647?ïëOAÉ?`!ÿ8Tá?dï°¾b6«?`!ÿ8Tâ?ï¦þGâT¼?¯w£å?†@njЬ?¯w£ç?ïâ'Æ:ìm?sOCt÷ß?mm9Å"$?sOCt÷Ú?_ÓN?‰z4Íe¯®?§…*âË"?‰z4Íe¯®4FGL J0529.1-2449c¿Èøц³¡ÈÀ<b›Zcù¥À:µ¡qÕ/rÀ<>ç;
H@‡0Á¾Ñ·@2ÙÏÏ?ńΆý‹¿£<§%Hcò?ÜjyMÉ·@Tgm˜Š?Ù©,߇¨¿çÑxÞc"9¿çÎ0_C\v¿ë]H~u|¿à@".þñ¿ïöÅ>cUNASNone$?ïþæz­)?!f¼
 ä?!˜U-nLú?!f¼
¡?ïýu´²W?T-ë€Z}?4WâZmJð?T-ë€Z'?ïåõ—"y?lLë_»?j
bh݆¨?lLë_»?ï÷õ†;ö?@U' Ò??Pòáˆ;?@U' Ò34FGL J0529.9-0224¿Ìi¹ÄƚÀ32 D®…ºÀ:}å‰\4´À;Än@O{h@öE)B@>ñ³/m@ӝ_÷·?êt™=SH@²ß­*p@ÕD¬à¿ÑGËÂᑿÆ|ÊÌ¿êw½ü¥X¿ïW}_§/"?Ñ|#ý`='¿ÆNxÉjl°UNASNone?ëýô‹"A^?ÁÍ?-á›n?À-Ñîú…?ÁÍ?-á›n?íy^$ƒ?ÆǯÐB?´5Ûã—t?ÆǯÐB?èhsì[|?´Áyn"?ÏÒ^0N'?´Áyn"?îvRüš'?°Èäˆ<)|?¨šÐ6W&ô?°Èäˆ<){4FGL J0530.0-6900e¿ï¶'üæòñÀ@:r2LƒfÀ7Öl9äþÀ;;¹ÿk@âQ—ø.Ð@ç±|å-í?¡š'_`D?•¦çÿ¶¸?öÛïqµ@±µ›ã÷?ìOu¹Nk¿Ô\Édb€(¿âµ†à‹P¿á×ÊÆbP¿á"€ãÀ.¿åpà<4dUNASNone3FGL J0524.5-6937LMC-30DorWest?î­X6Éi?¡Ån"³ƒâ?¥*|žSi`?¡Ån"³ƒâ?íŤh ?ÉRÔ£;l?·ÙÒÜ¿»?ÉRÔ£;m?ìy]úÉûÇ?ªZ›y!x?¼5)°!Æ?ªZ›y!x?è\žòÞ¶«?·Ne¬x?΍"4…%R?·Ne¬w4FGL J0531.5-7823?Õw¬·Ä›À>…'¢xæÀ:½ÚgüÀ<J=k›Y@ÿW±Më@QÁ"³¦‹?À1{¸ˆD¿°z_þ©z?ðÀÔÜeÇ@õpKAœØ¿Á© ã9öœ¿åø þ¿ê'%ëbd¿ã Å®¿åAÝ¥¸?ŠñTŸC
UNASNone?ïúaþŒiü?Gå«ñ]?FxÎXb?Gå«ñ^?ïüˆsAÙ?^°Î£'å??£¼eñ:7?^°Î£'ç?ïÒÀ&ç±?zÅ@ÌmÒ>?vöŸìŒ')?zÅ@ÌmÒB?ï÷ïDZâ?A¤»…õD?QÚ pœ;?A¤»…õ<4FGL J0531.7+1241c¿êè:H›FÿÀ&Ž·ˆ—é–À9Æ2Ôh£À;iÏûUvT@Š¿šàª@·V¾È'?ÐxR!5î?Öܒ½‡_…@ìÝÿ$7î?óᣖr¬?ǯ.–ÁM¿èrd×-©¿å—˜Ø©yá¿ë{Â)°¨¿ïû¤üۈ?éÛG¹ÒõUNASNone ?êk—v§+
?Äy±Q©?ÆQ¢%cS×?Äy±Q©?ã1ㅪ—?ÕÍ)'"`?ٜ8ôªÐã?ÕÍ)'"`?âK#Mˇ?¶ekÏÄ?ÛÏi¹dhð?¶ekÏÃ?ÐP5MFV?·VôOÌn?ç×õåY\Õ?·VôOÌn4FGL J0531.8-6639e?ï?Ì:KwÀ@K´¢3œÀ8ƒE§©ý•À;ŽÊw‡öÚ@ÚùªPv?ÿɌ;E‰?¡þ¾›B!?"‹|ÂÀ¦Æ?äˆô'
´@‡ÒFß8?¾
è¿×È¥`LEÿ¿áG
À²ã¿à+7GMœ¿â†òÍèU¿¿×Ôþ_
UNASNone3FGL J0525.2-6614LMC-North?ïÙÓ*Ú
?mx'ö®?sj'úòÜ?mx'ö²?ïHyB¼ô?±jvDÞã'?–ð׿èa˜?±jvDÞã'?î&¬"%z˜?¢¡.•Š?­•6½¨Vƒ?¢¡.•Š?í¾^Ìט¤?¡ÒŽq(2?²
	™C:ß?¡ÒŽq(24FGL J0532.6+3358¿¹:;Ûz?ÖâЯ°\TÀ9Õ¦k93þÀ;e·ÂyŒ´@Fj(ìç@'¼!ƒÞF?Îá\PãÈ?ÅФ®§?ö$SN[®?üÔ!s€¿à…°¾¤@¿æEMFÚ¯ä¿éùŒ|z¥¿ì}@"Ó¿ïÆa®pÁ3¿ïÿWƒuUNASNone?îæ¦]‰‹e?¤ßf]­·?¡•š'gI°?¤ßf]­·?ëð03Cå6?Ë`Æ")W?À??2ðk'?Ë`Æ")W?è÷zGŒÀy?³oäÛåºf?Ì"áÌþ?³oäÛåºf?ê _É[Á…?®Mà='C§?Ç~€Úùï?®Mà='C¦4FGL J0533.6+5945?¼! )e@,UîþOü˜À:‹øÇ&›À<Y>Y#@"yq…ÿ3@I©¿Š¯?ÁczcHyÁ?äF]²b¾@©†b…0V@ÐÎí
Š¿æSø`îW?ʊˆD1³+¿àKý"z¤¿ëÑ q$0¿ïÿ®2D¡?Ô¶0=µm5UNASNone3FGL J0533.2+5944?dØÿ'Q.7?hjµþÐ?ïë'Ø®Ò?hjµþÐ?…"ßՏJö?˜˜®]?ï«t€©ÂÕ?˜˜®]?›ã¼©æ#h?Ž×5eÚÂ_?ï â°Îå?Ž×5eÚÂ`?Œ¶|½Xvj?x¬	wOB³?ï&
ž'?x¬	wOB³4FGL J0533.9+2838¿ïz)		0‰À¤ì¦†çæÀ9@¹çíºƒÀ;!ÂÀ®@ƒvÐ@	ðÉS›‰?Æ*<Ó¿(ÆÚVM?Æè6 %#ü?ñ9"õjÑ¿á4PŸTÄ}¿åi¤ßGú¿ê#OÆðé¿ïúk _pÿ?í®/ªè¿ïÿ«±ÊUNASNone?ïëNZ­s?£&Ü5æg{?do±¥RŒ}?£&Ü5æg|?Ö=²?¨ùŠËŸ^?ŠJ`0"T?¨ùŠËŸ^?ì-,He
7?¥òæ‰t?s?¾–¼×–H?¥òæ‰t?r?ï®)`œ/?ˆ16"›{"?"u§Øô: ?ˆ16"›{ƒ4FGL J0534.0+3746c¿xq\"ñ6@4òd/UÀ9£¶"|#gÀ;c¬sßÌ@þ©éèß@ϒ¯šŒß?Í7ÿuÁx0?¿Þ-G#*?õ{¡çEô×@	©f®ƒa¿à˜›ò9¿çò³ç#¿çCKK¶¿çùš‹1!
¿ïûdŸç¼g¿î<Ö 
L	UNASNone(?ïû›uÀ2Ñ?N@ނm¿?A'(ÿ4·…?N@ނm±?ï¶n·.YY?®f¹Ã'?'dR4i©Â?®f¹Ã'?ïâ{÷89?"›–Ýu?ü?ŸC°øå?"›–Ýu?ý?ïÔø
é?b½oè¨?uõ¿yw?b½oè¦4FGL J0534.2+2751¿ëÐ/@Â~nÀyž×ÆûÒÀ:e:V=#wÀ;ÚØä2D @"&H?"?þ
Ÿu{­ ?Äã׫M D?ŽyÁô?ʧÓC3†j@0a"šK?Ö©Ù‰s²¿ì+º~¯•?Åû…‡hêz¿â©4wž¿è
ŋë›?Ö¸qËõ6xUNASNone?ïê)r¬o?eºK[¾?e֍Så'j?eºK[¾?ïøøË9?zžCÉÜ:7?LӋçÄ?zžCÉÜ:7?ï0ÈS?"f'5ð2?™ý&üõ˜?"f'5ð2?æð™?ORpmm?‰'[ÆCÙÓ?ORpmk4FGL J0535.1-5422¿Í"ÿT2¯À@XÍJ¡À:V¶~¡ÇÀ<LtÎ6/@ÁV-ßi@qËa'Â?È;v8@Ž;?͈Šèü®<@]GóÐG?þvyÇQ¿åèÅP׉¿èaÊsc¿ãèS;wG¿ä«Àb±%¿ïÿŸóOîU¿ðUNASNone?î˜f‰$Žô?¥*Å_F¨«?¦y—m·Í?¥*Å_F¨«?î`BÈc?¸…àM´ú?¯‰ûÓyÎ*?¸…àM´ú?ç×#Ÿ¸°š?²;¦:ô?ÐQ¸ÀŽžË?²;¦:ô?éžo•"?¯È•̒ñ?ɆC¡«­´?¯È•̒ð4FGL J0535.3+0934?ê3oÓº¾\À(@ÛH'ŠÀ:ìÏ¡"cÀ;•HFÀ®±@ÜѪF@¼mFTx'?Óœ"$'?ÝÝÒä>š@ko\¯-€@
kSù&r?Ñ{,܁ö¿ê5†öÿ¦¿Þ¤Cy|n¿ë¯
Ÿ$óÕ¿ïùu!j2ú¿ïüZžÜúlUNASNone?ï²qŸ`Õ?ˆK£Ü©?ƒc˜'ûJ£?ˆK£Ü©?ïbª?¯è´üG*4?"§¿ª½Û?¯è´üG*4?é¯Ðë¬?¬çOšÎ?ÉC¼¼SÑL?¬çOšÎ?î9KËj?"ó·ÒÏñò?¬kNO\?"ó·ÒÏñò4FGL J0536.1-1205¿Öó;ÚF•À6îיåÀ;\ÈWóÀ<†	g‡Î–@ K‹&5è?úV.u^Pî?֘"	\ ?å,Ýُ~@S1B˜+?üšÙ4ºð?ïÿë""i·?B;
ó?­x®ßÉK/¿Õ¬·¶Ì¿äTïE™¿ïþõU9UNASNone?ïñ@(E?e_
/)«E?]ׯußð?e_
/)«F?ê8‡›þ?ÍÇ2,cvÏ?ǥቐ?ÍÇ2,cvÏ?j,ÑU?›u.ª.ê?¦&)]2ê¦?›u.ª.ì?àîŒì¿?¹¼ë†I?Þ"æ'܁ù?¹¼ë†I4FGL J0537.5+0959?ë–^ûFT¼À&î™côÏÀ:#"D¾ÂÀ;œž%"ü@¥¾K°9@1·'¸¬"?ÊLå`íU®?Â*LDQ=µ?õ¸ÜÀ_×@"Äõ=l¿Ð]ó)®¿ÛëA,:¿î]©"â t¿Éíp†OåÆ¿åc¶ž78&¿ïÿöµšUNASNone3FGL J0537.0+0957?ïøIÔ~äø?S§&ԆI"?NØ®l!h?S§&ԆI"?ïý€lÐAÓ?T¿•çA´m?3ü™}ñb`?T¿•çA´t?î=ˆA,#?¢bËÄ?®?¬.÷{í=á?¢bËÄ?¯?ïòE—°¼˜?MjzB÷™I?[tО†Ñš?MjzB÷™A4FGL J0538.9+3549c¿ê7è0$º@x7~òNgÀ9œ#…}ƒÀ;'<ðKW@\лnÖ@ ‰…O_º?Ê2(œ+o?ÕO´þÏÔ>@é>›A?ÿMðbF?北'·Ôî¿ä‡%"Ï8¿á&caNN˜¿ê^á6çÚ¿ëE¿&ñÜQ¿ïÿm²æUNASNone$?³‡af(
ð?³®Þ>—N?íÓ:þ¢?³®Þ>—N?»ç?ò½¥?ÆÎãÕ<—›?샨K_?ÆÎãÕ<—›?ÅjÂh;Z?°W?MŸÁ×?ê¥O~åñ*?°W?MŸÁ×?³4ÿ•nS'?˜ñٙÔ]a?í™`
R5›?˜ñٙÔ]a4FGL J0539.2-6333¿íÊn=]%À@	d¾ÆyÌÀ;$Æ>=RÀ<Æ<üàÏ@<YC=A@0:û~'?Ë-‰ûìÊï?¬a´Mzª?âùaíÍÎ@zê,>¿ïþøÞ΂?ïØ#½Ÿ]S¿ë=nöWá¿´M"O£¿ä5o¸õs¿ïå`³IUNASNone?ïõÝ,iÇ? -å¸ÿê"?TE§×,r? -å¸ÿê"?ïüõ
'µJ?^D×÷xO'?8W«êU¶š?^D×÷xO~?ïÕ¬IcÝ?qò—ö'?u)üÛNf?qò—ö'?ïðeBž?R§dá'?_4ßzÃúê?R§dá4FGL J0540.0-7552¿Æ ÆɔÀ>•#¯1±À:J ˆ5ÄÀ<Kìåq	@95:õIn@V—kÁïú?¿ƒ˜%{:?Ì#îX^¼@

òzœ@	N'î['οt—ˆŒî¿×9_\±Ü±¿ä/µš &¿çÂâh?"¿íÿ8$3»ï¿¨'õ:ªúUNASNone3FGL J0539.9-7553?îˆ5àÔ)?¥ø"H>Œ?§|¡þ½w?¥ø"H>Œ?ïíè5§à#?,fö³o?bÊXÝ#?,fö³o?é.YOL˜?³6z²…ˆµ?˟FšÂͤ?³6z²…ˆ¶?ï'c¥ç?t˜W`‹ó?‹g†;½+?t˜W`‹ô4FGL J0540.2+0655¿ìÞ™'±À(Ü6q¬À:µ|8_ÂÞÀ<<3Ð$ë@!¼;ž½?ùcㄟ6'?׺àK}?ÍèþNe?úÔg–NÝ@[¹'ï?âˆö~vþd?ëȀB_¿âîà]Mc¿ÕmE	­¿ÈƒëÝ^?{¿äK™[†9UNASNone?ïïÔ\–I?b_J0×Oò?`+÷£i·o?b_J0×Oõ?ïûéٖR?\~Õ<]ë?@X™§Â´ï?\~Õ<]î?ï'xåË\©?ˆd;1rù"?‹aƍ(Õ¼?ˆd;1rù"?ïÓ½~ÆÅå?j_ðĬµe?v!@œÕ?j_ðĬµf4FGL J0540.6+5540?裗yIj|@)ægrÕàrÀ;u"ÁËèÀ<VòQÁ"´@s"à?@¥vjNR?Î7'^"´'?½¦ù>ì?ðÿfèle"@@o7›LÍ?íc\%šÄ<¿ÕgnÙ÷¿çùƒCì¾Û¿ç¡Ó#þâÊ¿Ý5ý''¿ïÿÿ)@k*UNASNone?ïýŒrI"ª?4KÊÚÃ!?3œm³Ú° ?4KÊÚÃ,?ïú8uAð-?díEÜ)P?G*ø?I§?díEÜ)P?ï®;6RÇ?¨½s¿ƒ?"q2k|N?¨½s¿ƒ?ïæ(‹ìWÅ?V·‡~ýaû?i×t¨;¨?V·‡~ýaÿ4FGL J0540.7+3611c¿ìFz
¤û@}úâ~À:Ç=@Ó/À;dS‹'@'Œ`÷@‰3¿Â?Ðǎß×@™?àtüÌnØü@4zøÄ¢?ù¢îA'šÈ¿ï÷"}~[?ïÏü'$y¿á9NÖ&é¿ì3шô/è¿ïñò¡ų?îÞëuUNASNone0?ÕvõM=?ÍæÃlþ?åDô…Ya?ÍæÃlþ?»,qf^?Ƒ³Ì.î$?ìš}ÑÞs3?Ƒ³Ì.î$?Ëс]ð¡>?³Œ`"XHÏ?韨ƒ×°?³Œ`"XHÏ?³4µs—!?£¢ÊfN×Ô?í™iQ|?£¢ÊfN×Ô4FGL J0543.5-8741?ÙgT5ߔÀ;ÈCރÀ:ÿƒ~`À<h30®ôu@M²³ñ߁?ÿžÔ¼…Vì?Úp™›&?ÁD°E­‰?üg+ˆD@×®7`iw¿ã}ú»×\¿ép|4.ö¿ß5ßJ}Ҕ¿Ø~ÿlÅ¿è9¿¾ëc¿ìA\[ðlUNASNone3FGL J0542.2-8737?ïÅ¿O-¤e?‡8Ññ¿šW?} Xi-͚?‡8Ññ¿šW?ïúÇ†?^—&ʲ ø?Eˆáçå»T?^—&ʲ ö?ïd³UºJ?'ÃÞ¢b»^?"oɕH¶¸?'ÃÞ¢b»]?ï¥ÜNyÑ?s
B"·ê?†¿Hìa‹ô?s
B"·ê4FGL J0543.9-0418¿»ÆóN2F3À0ú;%oüÀ:¬	æ~À;©Jß!c@¼Òo£üÊ@‰4\(?Ì
¾±:u?È·~Fï"@%cµ±þ@à™+µp?ï¿/À·ë"¿Ù­ÜÊ5ï¿éŒÏƒ³~¿ædËÇOh¿ïÿò"²¢?ïÿ9fS0UNASNone?î7äá?°/WMxRŒ?®¿®±æ?°/WMxRŒ?íâÍih¬p?¼'øõ?°é"´ºœ"?¼'øõ?çQwø2?¶Åw-d'Ó?Ñ\á›Þ?¶Åw-d'Ô?ìBü™®º?¨vrÒÎç?½ï02Š+?¨vrÒÎè4FGL J0544.4+2238¿ïÇZĜ¿ˆÀ3F~i'À:YËUÔGëÀ;ˆöšüp)@ )¡n@Ø
±?ÄóÈd2Y™¿±{PƒP,?ê+Xx`å?þ(V˜½üz¿ëþ¢1ìÞÎ*L…¿âÐÞßôǾ¿äXxœÉÏ¿éÔç¸á]~¿Ð³HAbJùUNASNone3FGL J0544.7+2239?ïE®ìNZ?–M2ºõ™?—^ê"v4«?–M2ºõ™?ï¾.#"Ð}?DÎù?€twËà½?DÎù?íL°³¼HZ?£¾6C½‰?µšzb½3?£¾6C½ˆ?ïé/'çÄ?Žn€ÓÂ}O?žÚ
£?Žn€ÓÂ}N4FGL J0544.8+5209c¿í‹hGƒz@''éÌ·ÔÀ:´4osUbÀ< ÇË)_@<Ä~¾Ý@õŠžT~?Ȥ֎—ˆ?¡ä´Âa[\?Ò6§|0R-@9ÌÕh¿á_ç@ìYZ¿â«Ûmi¿æ/Pà˜0¹¿ëù=í¡Y¿ïiОh‹Z?íÚ¤ü¤*íUNASNone(?ïÙ¹_ûš?xl1½"s#?s#Px³:?xl1½"s!?ïzšó?°Y}j;+d?¬¡ü¼T?°Y}j;+d?ï¤3-;?'֨х—2?^‹yšX‰?'֨х—/?ïÔ]@6מ?h¤Ã³žX€?uÑ_ä"1L?h¤Ã³žX"4FGL J0545.7+6016¿Ç;ÝÛ»bË@/yb(D€À9Êãv\}¯À<P•V=ú7@Hñk<¹ð?ýHÅ¡_`¹?µ–…=5÷?ӋÄY`Äf@çíA·Zu@Ç=˜^?ïïÑ|^ö¿À4âµÂD3¿Èô±ë±¿à¡'A5ª\¿ç«
Û%U$¿ïúo!ËׯUNASNone3FGL J0545.6+6019?šj€ýE2?˜•·==?ï,¯»ø×?˜•·==?…fb8Jø?'ñ?RwT?ïªfwÔ!?'ñ?RwT?ÓO´
=¢Ö?´Š5M?æX%ùa.–?´Š5M?˜½×1R?'óÃlÅ:Û?ï?TFv?'óÃlÅ:Û4FGL J0545.8-0905?ïÃ.+>À2­«ÀãŠ~À9Ó
ÙwÕúÀ;‰ùºk¡9@¥Þ^sS@Ð$ ?Àô+uúƒ?¡Ÿbûþ?ãÒácÝ @«ð¥oØ¿à~‹ì¿æõÊÝ^jo¿á>Nàð~¿äx6½¬Hs¿ã߃VR¿âñ+Pæ¢aUNASNone?ïä`Å
"?oP|Ó\l?kŸ:õü{l?oP|Ó\j?ïüˎ1 ?S¹˜oH'?9£Žvÿ?S¹˜oH?ïz‰ªî)?ÿ¸cx¬L?®Ê¢:à?ÿ¸cx¬L?ïÎ_¿Ù©$?hs`-C%^?xÐ +n?hs`-C%]4FGL J0546.5-1100¿ÜÎÿ!ÌEÀ3U¢Æi}À:a՟Ú%{À;Þ|2€…Ì@'Áºõà@"ÕN´™?Ñh·#˜5–?âý ⣣´@|FØ+¥ ?øwÛ¿ÙþŽÑ¿{¿¸Ù"ì
"οêEœVã;¤¿ì­Z˜¿áðk¢æIv¿ïùOýnUHUNASNone?áD`þõ÷e?Ð:©/¹©<?Ýw>6?Ð:©/¹©<?åUÆ6©É?Ó8ç…Ko?ÕTs"Ьn?Ó8ç…Ko?áKªÅŠh?¸^ýfõ2?Ýhªtë/Ç?¸^ýfõ1?܎â!™?¼íüÔR?Ḏï3}¿?¼íüÔR4FGL J0548.6+1200?ï']"øíÀ -i ­ŠÀ:3v†ojÀ;¿·lé7g@5XûC؝@³Ão1?ÏÚué‰?Ç6%ö4?ëÆxõµ#c@ú¨ïLÿb¿àóÛ>ªŠ®¿×ëD‡•¿êV¡'M¹¿éûibš)¿ï²Ô2ò›"?ÛǚþôgFUNASNone?ïR d­ƒ?®^¶byk?•»ójOœ©?®^¶byk?ïçH¾¤?"¸Í°x?~,[÷ ®e?"¸Í°x?骡ýZÈ?²?#ÔÙ|¨?ÉWéx
"á?²?#ÔÙ|©?ïª,3©¬Ù?u€Ö÷6?…tó"É'?u€Ö÷74FGL J0550.5-4356?áÏê>¶^yÀ<ÿ‹&9O­À:¯ËlÂÀ<™TÑél@@ }7Š…Õm?øàYÜë(?ÓOÎ>¼Ô1?Ïsû$y&?õÀ›€úfc@}hLðô¿é«ç¿ç4=õ.¿æ=•W¹Ë¿Â…"¿µî¿â·{ây‡U¿äkg†ø­UNASNone1FGL J0550.8-4400?ïú8ج'ú?Cçi¯t½Û?GO`B?Cçi¯t½Ò?ïü`5‹?XìŽc´??üþS£öÅ?XìŽcµ?[ÚÙ?‡Ø»=â&0?‡yé	Iê?‡Ø»=â&/?ï×P9eYü?e#vá<SÚ?tWãMS?e#vá<SÖ4FGL J0551.7+0446?é"e¡AãÀ%î°t§qÉÀ9±*˜YþyÀ;…ùTTK@{"úX¡@4"Dž?ËO'ŠÝ>?á Þ'ö @w"}Š@£tvŸn›¿Á¯…,пÝ;%û'2¿ëC–ß~*¿êï/}œ
¿ð?ïÿÝe¡D‰UNASNone1FGL J0551.6+0449c?؇¹ÿ§}¸?Í°¡vý˜?ã¼#,A%?Í°¡vý˜?Ôâ/'Ü°>?Óý˜ËÐ>‹?åŽèl§á?Óý˜ËÐ>‹?ß}uø‹?ºH¡ÁÑÐÂ?àyÁEvƒº?ºH¡ÁÑÐÂ?Înö¥úÎ?¸º6òî)¦?èdBV¾ÁM?¸º6òî)§4FGL J0551.8-2130?îUþcöæÀ6Yl6KìÀ;jlËÛ5EÀ<°IpŒZ@%8ZåS×@1¡šïÛ?Ñÿƒ
6?Ëàs±B?ö"ÐÜüÆ@â×P3t?î3Îc¥ÁÆ?îšcX"쌿àMªx.—¿êå"Ï7á¿È/ïÜÇ@Ç¿ïÿ~À¥L*UNASNone?ï¿JÌ«÷?"P›ˆ'½*?€?­LÕ?"P›ˆ'½)?ïó©çÓB£?y	é,j`T?X¬0Yzºõ?y	é,j`U?í²þë–ÂÖ?¢m"_[òH?²h£IéQ?¢m"_[òI?ï¨Öê|h?x«pjhÝ?…ÊX…`å»?x«pjhÝ4FGL J0552.0+2656c?ï–•þ?Çh'œ&;ÔÀ9—ž™ À;8ûefŒ&@›Ñ,Wø@[œ›¬™Q?Îb~ºÆ?Ú	{>d¿?ø¬Gõb?ò?߉=¿ØAN^²½Ø¿ß1BªŸ{¿çeQÉ oâ¿èÊ/cšÚ¿ï.mÚÚ¿ï;^g"dUNASNone(?çCÌёÿž?ʈÀ–ê]{?Ñxf\ÜÅ?ʈÀ–ê]{?èÜTp¼Ÿð?Ó?ÂáY?̎®=
€B?Ó?ÂáY?ⳃ¸è—?´îÔܟ²ß?ژøà.Ó?´îÔܟ²ß?á"îW¹Î?»ÆÁsÃLŸ?ÜÖ#PŒcÔ?»ÆÁsÃLŸ4FGL J0553.5+4810?è8ðó.¶‹@&HƒýP"À:—Ò+ìîÀ<¾mŽxÔ@Ö!·4à@O–áXu?ǁð/¨d?FÚ
Û¢¾á?ÿ	"=—¿å Ã6iI¿æ@š>Û"¿ì¿†]|²Ù¿Î£¼ÞLù¿ïÿýF\I?ïÿÃÏÎ	
UNASNone?ïíô¦"ö ?É¥~h¾u?bY{	`$?É¥~h¾u?ïùÕ;^—?¶XŒOðî)?œ€ÅX"-7?¶XŒOðî)?ïGÎ`?"½P	$…ë?7Æ>sø?"½P	$…ë?ïê@û[Ú?^í¼žì"?eú¿¤%º?^í¼žì"4FGL J0553.6+0100¿Ü ìqÕĆÀ(¸mµ@æÀ:jíLŸÀ;¶3PdŒ@'Ù®¸»@ß	zÓõ?Ø^K¥Dóz?êCXz™@H¼¾aÏÿ?ý‡¼!ƒÞ¿Ð¯9¾èˆ•¿Ú"ã"Ê*¿è0‡‡H^>¿ï¼sÿP³?äJ
M{¿ïöÿ<
ÈUNASNone?á!•ƒ~t]?Ðn`¶œA…?ݼÔùE?Ðn`¶œA…?å׃‡#?Õk‰÷éû?ÕÎQÊøñº?Õk‰÷éû?Û²'"À/Ñ?¾Y²M²?â&¾µŸè?¾Y²M²?ã®r™FÓ?Í0þ˜Ì?Ø£ÍßrZ?Í0þ˜Ì4FGL J0553.9-5048?ê-ý¾o§À=ˆ2¹¯æÀ:æ9ïôÀ<³ªÉlÆ@s*ÈU™º@«`¼z.?Ë{O+·=ï?¹o0'ˆ?í
Ž>F·Ÿ@S—ÖJúпä¼ò.†%I¿ã—¢^S*¿æ»ÀÖ…&¿Âf%cf×¥¿î
?¿2°V¿ï' 
UNASNone?ïü"Æl?7?MRûF?;gÌŸþé?7?MRû*?ïü/Øhxª?jŽ®?><¼:¬¨?jŽ®'?ïÊÓST?€»X³Yöb?zþVvVw?€»X³Yöb?ï砆kB?[Ë€~{?h_y锾?[Ë€~4FGL J0554.0-0839?éÁ¦5;À0§õƒ¥À:yB¾ÁqOÀ;ú¬ûv-"@€ÝŒb¤e@ÿñQçSa?ÊÒ¥û|¹?À–Dû\­*?ôGòø°€f?ø>3i¹×þ?ïÿ*bT3¿ÝhLðô¿ãÊGÅwÄ¿âÅaôfſ揉	ÿ]C¿ïòd6
~UNASNone?ïç̾¨Õ?k¤qx`ÀÈ?h3AðW+R?k¤qx`ÀÉ?îmßQÓ8î?´ÔÎkÈT4?©"
âÌq?´ÔÎkÈT4?ïˆpÙÆ?"ɜ¬€?œÎñäÇ?‡?"ɜ¬?éäHQaV?¨#"‰?ÈnÞº{Σ?¨#"‰4FGL J0554.2-0259¿¼BðÒ&cÀ,'gn¤"ŠÀ:>zt:d€À;¾G^cb¦@%ï6¯©@ys{øžã?Ám6åtÆ¿ŒÃëk0™?ÌGԪ矷?þN9Vé?É@ˆÆ¸‹¢¿àqöó4¿í¦ÉB~ª«¿âê®ñ𿑶N[,Ìg¿ãêJŒL˜UNASNone?ï}i'ø<?ˆ×>/N.?RÏ ø}Ú?ˆ×>/N-?ïúÐϼ'?hǬÉ6]?Gð¼Ác?hǬÉ6^?î®	Z]#?˜¬ŸÁ¨Ã?¥jZ-Æ?˜¬ŸÁ¨Â?ïækù ƒ7?[åzõ·?i"ß|Èc?[åzõº4FGL J0555.1+0150c¿ë…h´N¤øÀ'GLnm›åÀ:F¹"À;£)¼'ì&@úîãøãV@ŒT6¸ú?ÎÕ1J?á@B,Ja@Çþ0òç?øÇøâªY°¿ëL§ãß8	?ï·C[Ÿc¿à;Vƒš¿ê=sº¿ïÿýç!é¿ê]"°§UNASNone ?´µžûÁõ˜?»ªèœÛ@$?íiL ‡ÁN?»ªèœÛ@$?¾üT;É·š?Æú<<Ú/?ì ux†É?Æú<<Ú/?³ë7Yu?¡í‰å%<?휢™ݲ?¡í‰å%;?ÖàWѳ&?yS"(-?ïyHýArf?yS"(-4FGL J0557.5-4452?îS¼kV÷À;óìþ›{òÀ:g%¹Íì‡À<NØúØ@êç§Ä¡@t¹­6?ÂSÕÀ{ο Ş°.Ü?׍ÀÿA@špkø̅¿×@>^Šyì¿é2"²¡¨¿êÈx	&o¿â¾N"ÈQ¿ïþ
·x§²¿¶²$ÀS UNASNone?ïþòd+¸‡?,l°ojÔ? Ù½Dw˜?,l°oj®?ïíђ?Ñ?~Ñàɛa%?b.mÀà/°?~Ñàɛa$?ïÛî|ÚÊ"?uZwÆN*¦?rÁ'šïL?uZwÆN*¢?ïôÅ<Ð?JИâ|?Vu‡Ð`d?JИâ|4FGL J0558.1-2113?éþ"^üýCÀ4à¤ãy·|À:USʂo±À<jT¨ÎÀÃ@¿(Y@ˆœ|&Â?Ǩˆòß[?Ѓ­Ÿ
ã@÷9zu$?ýs$ºÊl?ìO"¢—D*¿ÆjOv`¿å—ö+jçտݗ|ÞÍÖ7¿ífNžHªê¿ïÿߞ¶ŽóUNASNone?çl‰ï?Ýž"?Ñ&ìä!Ïî?Ýž"?éå6ÀDi?Ë^ѤGtc?Èk'ìþîZ?Ë^ѤGtc?æ"4)Iԍ?³lÅòu?Òח­lVæ?³lÅòu?åÆ'ƒÍW?³×·úší?ÕÂs°øeQ?³×·úší4FGL J0558.2+0132c¿Ø%­ÛcTÀ&/¢ß"xîÀ:?ûUvTÀ;¨
^u×@žÒmö} @ÉzUý?Ôæ‰ah$×?ڄKßQ‰µ@
;3Úøßz?ÿ†xÕ~Í?íµ"Ód—¿ßƒf|`΢¿ç•jËOõ¿éŽ•¹:I¿ïÿÿ>¹ú?ïc!u´UNASNone1?éKÅ©94?Æõ8•$«?ÊÐé[/Ã?Æõ8•$«€?á5â±9?ÔVƒÿ!­?ݔ:zÁ?ÔVƒÿ!­?ÛãòwúMº?¸÷g‰
‰ñ?âÄÙ#?¸÷g‰
‰ñ?×G¼ÿ•3?¼È}Cµ]p?ä\!€z5f?¼È}Cµ]p4FGL J0559.3+0352¿æùõq3½À#"Š½]ÄÀ:	-ãÀ;±6½+o@µðöøš[@-¾Ý '?ÕE~ð ç?ïÿ› 'V‡@è+}\L1@¸PW†N¹?ï[Û]‰H¿¹C`Á¥–¿îFÄ	¯¬+¿ìÇæîð
¿ïٓLØ ¿èñ$?¥\pUNASNone?Ö¤Růn/?Ïp«ë€~?ä­Ö(Hç?Ïp«ë€~?ÊNbPÀfÞ?Îz½¿˜LB?élgkÏæH?Îz½¿˜LB?ßg{šû)?ºŠª7"Åš?àLB2'pj?ºŠª7"Åš?®ÖÝ@ˆTô?œµŒ…­X?î'+÷z°?œµŒ…­Y4FGL J0600.4+4949?ïÃØfûÄ@)ž™Ç¼Â"À:í¶ÓfDÀ<Jž6·L@ _Ž…ê:@´Å¤º_?È{T44ºó?¥S°ß¹ìÿ?Þ–¼f@Lyð'οë(øçÝÊK?ì*³Éƈ¿î\.Õ?ÆÐ{k0P¿é"3É[(E¿Þ¦ž9çWUNASNone?ï[f8ŏ?—ÌY•J?""8ç_./?—ÌY•J?ï·UÙ¿%V?£äõ®l?'*‰6ª ?£äõ®l?îã֘§³¼?•NßÚ)á?¡Â–u"Ä4?•NßÚ)ß?ïӕ8,9?m+ôwŸ;I?v5céøcT?m+ôwŸ;G4FGL J0601.0-1016c¿ïN<»¹ÀjÀ/žj±NÂÀ:XÌ'©»À;žøÐ`Ö@¡di6$@
X³ö<2?ÏÇó^±ç?Ü®W+`@ü¼Ï(ǟ@Ñõ!T¹k¿Æ°(|Jÿ-¿ØiP{˜|¹¿æ£mùÞý¿ëá¬Bh°C¿ï÷íA·Zu¿éˆ²r®sUNASNone!?ìTjÉñì?¹òÔo‹¡?½_T©°pª?¹òÔo‹¢?íœtÁáZ?Ã÷êï\ÎÊ?·sYðõ1?Ã÷êï\ÎÊ?ä(zÔ&^C?µ$;ܨ¥?ׯ
W³C{?µ$;ܨ¦?ëð7qX%þ?¦~‰·bäÜ?À?":Ÿh?¦~‰·bäÜ4FGL J0601.4-6057?ï1Gh8YìÀ=|MüãÀ:ò{+‰>À<'é]ýY@¼úh;~@VÁBU&?ÓBýwºw?ÒK!{û£û?þZ%zãËí@¥Šeôül?ﱚa•œ4¿èHâA©¼¿ãtŸM ¿áà1~'ML¿ïÒŠÝ>4?êpYddIUNASNone?ïÓv£û¤í?|p.žì?vD®-‰¯?|p.žé?ﮚáÿ¾?"ðo$ت
?"Y€Y?"ðo$ت
?í H˜³Žç? Wÿ:ï`Ø?²ý»:cˆÆ? Wÿ:ï`Ø?ï›Ä­FÂ?Œo#Ai^Î?œŒ‡jW'×?Œo#Ai^Î4FGL J0607.9-1904?ëK è¢åŸÀ1쇇H^>À;-ÕctCŸÀ<Û®ïl@ b¸¬.q­?ÿ{ ÒÞ^Æ?Òâðe-VO?¾æÒ1›Ä?êÔë´ï`v@l´S"6†?ç¤ÂAÉy¿ídƒ¢·O¿â8j_oQG¿×Õ'¤´ªÂ¿ÝpĎ9ê¿ïÿ'þKÊÚUNASNone?ïý"Ë­Gð?0RQ0ö?3a¢•À°?0RQ0ö?ïú%ñ"(?hg©Ûù?Góh;wa?hg©Ûö?ïé#´`d
?p •bY†¹?fÜKŸ›õ€?p •bY†´?ïÚ6ŐU?`§w0Žz?rä7Õt-?`§w0Žz4FGL J0608.6-2305¿î£÷ŸŸ^ØÀ3SÐÚèÀ;LÂPrÀ<ˆœC˜E@ápÌÚ@‰ë têŽ?ыÝÄ@â?ÕHK=–
ž@¦±\.?ôV¥‹•Iÿ¿è8Eáá†î?ÌùÁâãåm¿ç=|'‡"C¿ÞùŞ…;¿¿ïÿÌ3IÙh?ïü,d1UNASNone3FGL J0608.2-2306?ïº[ò½ º?"ü;çö7<?iP·Ñ˜?"ü;çö7<?ìí ‹%ìb?Ã8‰Uë?¸–û¦Ðœå?Ã8‰Uë?ì›4²]D*?£û"žXɲ?»&ZmÞ±?£û"žXɱ?ènÈÀN?¶;FŸ¾?ÎDÜÿ²Çª?¶;FŸ¾4FGL J0609.0+2136c?ì6d}õî?ì'ÔžReþÀ9·¡I'CŠÀ;F"ôï*Æ@itû)¬w@
€™îS/?ȑ)]œhV?ØLv›gÏó@ê^ã»&?ëKÿ‡V˜¿ÓmˆÄŠ3¿â²âÀÔñß¿àJþ¥·à¿èÙÇÚñS¿ïþAÿ©ÃÞ¿ïó÷H¡YUNASNone3FGL J0609.3+2131$?ÔâkºŸ±?֊(ð>@Þ?åŽÊ"°?'?֊(ð>@Þ?Æû"; $9?Ò¥Gõ?êA7qöò?Ò¥Gõ?ÌÄ='²?¯=·´1•?ëÎð¶Ó?¯=·´1•?‡:b ©à?rcynl|?ï£u}Yø?rcynl|4FGL J0609.0+2006¿ÎoºRÑN¥?Åd†gbºµÀ9i'¹'m-À:õè½ÄM@¯r2!I@z¼i¨:?Ô;âjØ?ã]0'oí@³?…Q
9@¯upðX¿Õ1Ä{¼¿Úâ;Þ}y¿éC¿rq6¤¿ë*†ñ÷(Á¿ïÿåþÌú¿ïŒbUNASNone?ÝúP¡ÌäK?Ô:Ðÿq…?áׯÚ?Ô:Ðÿq…?´""Û3êÐ?ÄÊoX.í&?íom"™'¦?ÄÊoX.í&?Õ¼û#ª`?¶ï_väÏ?å!'1n*Ï?¶ï_väÏ?"ļ¼J!?pÄÌà<tB?ï¬ï•
×?pÄÌà<tB4FGL J0610.8-4911?è£Ó͉7òÀ:–YòºÀ;˜=Çá¬À<Ñqk}&œ@!A'±tט?þÐæòèÀH?ÌåÚ9òÀ?q£x}…µä?«ÊD /9B@=^Wú?ï饠ÿˆ¿êŽß+t"¿äHZ!^Ÿs¿Ì‡ì]‹ÌQ¿êk[˜­
¿»€@­S8UNASNone?ïÿŒ	ÐÍ?	ܤ•ÍQû?ý¹K̽È?	ܤ•ÍQ,?ïþd¯ß/'?VƒÄ,Å«?)µ
Ûs?VƒÄ,Å«?ïä®=?uåȦ–õÎ?kQýçÂñÿ?uåȦ–õÏ?ïûz«	c?5la?`?B¡SÚqã?5la?Z4FGL J0611.4-4722¿ëþÕVžÀ:ÇÚÄçÀ;‹ûZu—À<¿a¥6†@ý?Ãdn?@$	å\Ë?Ó«ãH9Tµ?Äï"77y¿?îü®a|ǧ@'Góߋ@?îâ<À县ãØöT…"¿Üß|Ò¹uØ¿èDÔ «±Ÿ¿Ð6ɀ<%u¿ïÿHµ{wpUNASNone?ïû›h_)?Awe¼X&?A'_'ƒ]1?Awe¼X?ïþdÈÜ×õ?K\ƒez—?)³r2€¸è?K\ƒez?ï±öÕ›Õ?}r*ÙÆ?ƒ'J¾Ù
Û?}r*ÙÄ?ïõQ6¿Ó?G'1n©YM?U]'ä€Z°?G'1n©YG4FGL J0611.5-2918¿ìé¤lÎŒÀ4ñŸŒ¨À;:Z—%KÀ<¸'MKã-@O'M ð@¼ù jn3?Æ
)#ºÅ8¿"zÞåËmÉ?ÐQJ8ˆ@!SYÄAŽ¿ïÿ_Dä?ïò$	ʄ¿èL?^9Ç!¿áŸ©³`ë¿âø›AåR«¿××Àâ¯bUNASNone?ïýæàW??2†€Å ?0ÈýCö ?2†€Å¨?ïþcýûóh?Lm­÷eNu?)À @Éw?Lm­÷eN\?ïáwûé~?r¤Ldo¦›?nˆ€¨?r¤Ldo¦š?ïüTqÒß?1-NúÇ6?=\qi7?1-NúÇ4FGL J0612.6+1520c?ïÊX5Õ3#¿õûš—À9Òc+Hƒ'À;$ý
':@jüz9'@'BÛFã?Úð¬¥åØ7?݈Vü1Q@ˆ.›
³@ŠJÇ#–?ïiGâlÇ)?Ô¿tŠ˜¿êrÇ2Y ¿í¦grÕàr¿ïüsž]M¹¿Fz•ÈSÁHUNASNone ?êr-̖lw?Êœ›Û—`?Æ7HͦN#?Êœ›Û—`?Ý©žhcÁ?Ö ¡QiZ?á+w0ËÎ ?Ö ¡QiY?ÜC3qæ=?µT¨K¨ðë?áÞsæGá?µT¨K¨ðê?¬pzCËø?™Xďî?î8ø[ÈA?™Xďî4FGL J0613.1+1749c¿ÚûU,!9M¿µ¿¿¯>-À9T*:†åÀ;dØǬÒ@ˆuÒ4j@
0'|G?Ã1U¡Îò?´Fˆ"ùª?ñÓÿü¥­@˜,J¶²"?îޏ¢ŸÒ™¿äKb¿gßb¿é¶nfÔ¿éÔ¨c`øh¿ÛÅÓ~—µ"¿è{éOºRwUNASNone$?îorÞYB?¦Pïz‡t?©Òúká?¦Pïz‡t?îÞþD1
º?¸Ðû#Ÿ?¢¼ï$J?¸Ðû#Ÿ?ëÄsÞ'm7?°:~³\­?Àî0‡bK!?°:~³\¬?î!œÊÉt?˜¡3˜ìSK?®íæ3ShË?˜¡3˜ìSL4FGL J0615.9+1416?Â^4¡¿òê1ç٘À:!<ªÀ;€Uu}ZŸ@©®Œð¾Ä@sÆßî?ÒMyšöë?à/‹^¿@
9™Üµx@`¶™Y­Æ¿áOuž'§¸¿ã5­–¦ ¿âöT…"RX¿íχ\€3—¿ïþÚH¶R?ïùv
£V²UNASNone?áEµË$?Î0£Ÿ•?Ýuü"i·Ö?Î0£Ÿ•?ã²·Í?Õøøf'ª3?Ù蚑Øeû?Õøøf'ª3?ҁdˆåN?¶þM"Äâ½?æ¿M»¿
Y?¶þM"Äâ¼?× '<N2z?½ñc7ƒz?äoìaØæÄ?½ñc7ƒy4FGL J0616.5+2235?ì"$²[@=õ~œ¾À7ÈE`\a*À9ÞÅFƍî@"ϝ"úh@R¢™ó[­?¸–¾»<,?¬ø@¡Žc8@ÂJ»5'@V¸­¿ïâ'x?܃ÒÝÝì/?ï^ˆ¶óF´¿Ú%р´¿â#πÜ3¿â"@^"àÍUNASNone?èÚ6øt@‰?Çõ1"Z+?̗$.ýÛ?Çõ1"Z+?êU_j¼?Җi¯æÙû?ƪ'U
¿¨?Җi¯æÙú?åÞvÖ4?¹w»Ñì|?ÔCáúS™?¹w»Ñì}?ä<sŸ
?Ç;÷ÑjBE?×ۇÁëé?Ç;÷ÑjBE4FGL J0617.6-4028¿îø`Ì +À7Kğס<À:Y:Ütà}À<Aß®Pá@"ÁlFz8@²c/
°?Àâ2d¬'¿~9¡æܐ?´Œ•z%5@¿ê»Ë?èQ­DqI¿ã–ñH­¿éŸK¿ñò÷¿í-­LÔÄé¿ášß÷-É¿ïýVlô!UNASNone?ïÿ²â'f?¨Û^ÐJ?~‡[f¬˜?¨Û^ÐE?ïþàÄ¿t?B˜p2yß?!ó¿Dʉ?B˜p2yß?ïÐ"|m?~ÓúåƒÃû?wøwµÁɳ?~ÓúåƒÃø?ïÿ¸zÍ©>÷³êš¸à7?á{•Î¾>÷³êš¸ß‰4FGL J0618.7+1211¿ì¤‹}bm¿ùvœ>ˆÀ9Žé#D¨¦À;G5>¦-ý@ʈzdØ@5½ÿªo«?ο<"÷?Øwîý`h@ëð«Ï?ýÏôÄã¿ÒÁÞݢĿâT‡@сg¿ê±  œX¿ïþ†¸ìE8¿î{qZ¶.ü?Þ>;Ú¡¡¦UNASNone?íî}s"–å?µG¯ÍÂ?°Œc[HÙ?µG¯ÍÂ?æYèôâÎÓ?Ó;¿t?ÓL.:bZ?Ó;¿t?â%TÄ,|ª?¶È°ÁºøÞ?ÛµVw§¯?¶È°ÁºøÞ?ÜÚË=_!?¼òùB?ᒚaPup?¼òùB4FGL J0618.9+2240c?ég"*B}6@díoڃoÀ8£$G%ŽÀ:V>hñ["@ä-;¢m@0;>šo'?υŠX‰?×E$>MÄ@h›€úfc@ØçÓ
ƒ¡¿ìŠÝ"3¿Ù_`"T"«¿Ò'¾+I¿æO_žÌ'¿ëá'fw-^¿êœöElUNASNone4?‰¶ýžüVµ?œÆ´ãÄ4?ï™$	"¦?œÆ´ãÄ4?"º³Æ¡?¥æ*k5â÷?ï_Ê*aÊø?¥æ*k5â÷?¥ˆ—˜†Šò?"\Õ®'Ü?î§v†w—Q?"\Õ®'Ú?…¸}+èƒ?x[½7×B?ï©ÉP^?x[½7×C4FGL J0620.1+2246?èÁ÷î%k´@
º"¹À9W|i+À:ðÁëÈ:—@!`>Æ4W@F$<jÿ?ÄK©â,£?°Ø*ùÓÁ?óR¥ôñ¯?öí՚¦µ¿ïðÏ«¤^?ïÿ}ÄPýI¿è¦,Od¿àcuÏ¿ì×LbY;†¿±²à<–3^UNASNone?ìü^æNP?¶q¦7Œô)?¸%͍~?¶q¦7Œô)?âe½Jy™?כ¿Úl"¶?Û4…kÍô?כ¿Úl"¶?éMY
¨^¼?±2ˆWQ1?ÊʛÉ^…?±2ˆWQ1?ÕúÁ‹¤6?ÃYkŒq*i?åñ:-ä?ÃYkŒq*i4FGL J0620.4+1445?¦ðÊ¥ ªG?l`ÃËW"À9ªu߀-¸À;LM++ýµ@¸¹Å^@F&}BJþ?Åʤ¾æ°#?¼X̔m¶?÷pd·9½'@´Áº ,?ïÌÝÉtR¸¿ã¡fµN+¿è=Ëݹ"¿ç_™Ã‹«¿ãË£l2›¿ïÿ!}ÿ	`UNASNone?ïÜy1M,×?xÎCGÛ¨?qÃgYi"á?xÎCGÛ¨?ï{Ó2刮?°æ›Áˆ?…™£Nê2?°æ›Áˆ?î©Cœ¹cô? ¨Æ¸àӊ?¥kÆ4iÀ´? ¨Æ¸àӈ?îüŒ$)B?…p<º¬*t? 7ç=½ká?…p<º¬*t4FGL J0620.7-5034?×®NŠ¥ÔÀ9Q—ÃքÀ;•æR¯Ð=À<ä1Uãad@!s?Lœì?³IWaæ¤å?âøVCæ?ï÷q@ŠØ?øAÔ¶¦@J=g>¨‡¿ïùæÁ²À?ï}4ßݵ¿ëG¾Ûr'¿ÏkZXæ÷¿ÓkÁ¹É:¿é)g7F¾*UNASNone?ïûX".ԓ?C–â¾"¿?B¯D­³y?C–â¾"É?ïþŠõð{?R65ÚÆÓ?.gP øVÝ?R65ÚÆÝ?ï—izæÂ?‡VÂþ+ò²?Š%¡FO~f?‡VÂþ+ò¯?ïþ³½þŒ'?*®éti—?$Ä 6÷_?*®éti…4FGL J0620.9+2201?¾¬úüxá@/ !·"À:íFƒrèÀ<º&‰@$d/€ KÐ?ø÷3"«C?Ǽõ©ºÎó¿ŸÔ€Âªk?ÕQÓ1jÜ@Vô²ný¿ïÏJöžWn¿ÐÐM_Ú08?ïývþ«¿èÁ€}éºÄ¿Ì"O
TAÌ?±£až²UNASNone?ïÿ;¢Ê?!* ³³Þ?ŸŸË¦ãœ?!* ³³Þ?ïîŒG¹‰?›Tõ?&b?as¸Fûv'?›Tõ?&a?ïÃq1¡Ð"?€
ú.Œ	}?~Gg/ï1?€
ú.Œ	{?ïùn¢ân?J!ʨÅ	Ç?KòEtvFô?J!ʨÅ	Í4FGL J0622.5+3120?íV°ï7w@ K£ÂˆÀ:*3°1À;»©É'†@¦",0‹@žÜ~ñw§?Ñ`šŸ~
?妟Ԝ$@âZÛGº@ÉîvÚ?ïÛ·`Ô×?åå[¤k"³¿ã¸¥bûwÛ¿í͂iÒ+±¿î
^þ"¿ïý'AŽ?ÉUNASNone?Ö1Oðúëâ?ÊO‹á|î?äçX'Š?ÊO‹á|í?ÔOÂã]tÅ?ÒQÞÛ¨µè?åØŽQEž?ÒQÞÛ¨µè?Ú[Ã`¶ý?¶ÓtJ	G±?âÒ{Ϥ?¶ÓtJ	G±?»šß?A?ªoð|Y0Ë?ëQH0/œ?ªoð|Y0Ë4FGL J0624.7-4903?îؑԑ"€À8U»YÝÁèÀ:Õ}<kÁÀ<…´Eâb@òàY@@×Or.Å?Ð^Wú?ÔXsÉü7ô?þø_<¦y|?ÿÃVçmb¿âC"×ü¿Ü·ØIё¿ç›ÁýeñÌ¿çè"M×ú'¿ð?ïþª*
•…UNASNone?ïæzñ<¯?w]rd°~±?i…æÃQ7?w]rd°~°?ïy˜0WW!?¢¨Î¤L;?Ìùõá?¢¨Î¤L;?ìɕèô1?¢0z¾>?¹³P¸^wÕ?¢0z¾>?ï&"æ?'žT°1éç?Ÿ»<Û¼c.?'žT°1éç4FGL J0625.5+7029?íy[bÃÈ@7Y±ú¹o"À;ªçä€G¹À=µj°x@!jÄ@?ú±´"#˜?Ô;CMÄ?ÊI¢¶MÚS?õ‹Íþûô@‹=8ÌÛ¿ïÿâÙ~‹÷?ïÿúŒ—Ó¿èÞ*o¿yî葵†¿à]½Ž–[¿åª[Þ£
UNASNone?ïûY…Ÿï'?A+®XcO?B™é€A·d?A+®XcV?ïùø5҅"?f»"Ž"?H(µë|t?f»"Ž—?'Ž?‡-åÅÐó?‹'»<ö`?‡-åÅÐð?ïӚS¼œ°?h%YºKiB?v2Ö!±¨J?h%YºKiA4FGL J0631.0+5626¿©­A	嚃@3¥õß덂À;-DÏ<é•À<ÁŽêéîF@çÁÑ;?ÿúü‹z?ÑaæåQÓÝ?ӗ­µ°@Á[šZ‰¹?þ²Í‡²¼U¿ïàîzÔ]?ïF"y&²?̃K쓿Þ>˜â9›'¿é6Í0ŸÛ¿ïÿúŒ—ÓUNASNone?突@»¢?ŠÀŽå²?…š¯ú"?ŠÀŽå±?íø4_Ÿ¡?À·#0)?°>]ô?À·#0)?ìßp¨7y›?¥
C)´Ÿ?¹z¾D3'?¥
C)´ ?ê%Ì'ê?ªßØÖTPä?Ç£hÏaÀV?ªßØÖTPã4FGL J0632.7+1215?Ú1{ØÚU?÷¦Kç_À:
á'ï¤À;†}=B€®@"'Ñÿ;µ@&eÅV·?Ëc¬¢µÍ?Ô
"þLf@	"•á~4¹@ƒwçî¿»Tÿá¢ô¿Ïxbmοæn'¾-øŒ¿ågµñ¾ô¿ïÿþˆ0»Š¿Ì<Vžó UNASNone?Ó·‹éDR?ǀÇr\‡ï?æ$:p‹]×?ǀÇr\‡ï?Ýp܋ßú×?ÕY™ëô?áG'º"?ÕY™ëô?ÕUlùeå?´À¬°Ò´Ï?åUIðM
?´À¬°Ò´Ð?àÍæ‡{b?²hZØ?Þd2ñý	;?²hZØ4FGL J0633.9+5840?ì;™ŸÝ@4¾™A…ŽÀ;dûHábÀ<Õ±·Ÿ@ 	ËÚŸŒ@ÎÓš3ó?ŧ`Ÿý·?À­ëÇJ?ÂQœÀ? ª@ñ,}ŒrÀ?ïÈW¢~D©¿àW@Žeˆñ¿ä t´Ý¾¿á I·6ì¿ß‰ˆª^ü¿Ô´4iq3UNASNone?ïõ_ÃïXö?PGÆý€•1?U@x!Nã?PGÆý€•2?ïüWZhŒ?[ùÁï)ø??E,»œo?[ùÁï)õ?ïèň'°¼?o?m¢`âÁ?g:wØOCÇ?o?m¢`â¸?ïâq¬àkz?Vݎm'¡?mŽS"†Õ?Vݎm'©4FGL J0634.6-3046c?é¨"Eã«À0Ï8£µ|NÀ:8WšÀ<DOúêŠ@¶Ñ"@ÈòZ%"?ÃyR¼»\¸?׏=Ë·?õ#ºð+w@qµ_ðý¿¾²»(µ€Ö¿å«;þ/¿ì¥• æ"õ¿àê¢Àß®§¿ê˾ßK¿ïÿøÞ£ŽæUNASNone ?ï'Ÿ
+b?"'¦dró ?~˜=u'U?"'¦dró ?ï—©ó? µaæ†Yß?Š?øUƒ>Ù? µaæ†Yß?îs)UŒ¡?G_/!ˆx?¨Íj§6%ø?G_/!ˆy?ïV·×Ý$?ƒ;¨"Þ·?•)ä[Œ?ƒ;¨"Þ·4FGL J0640.9-5204¿ì]9ŨMÀ6Ÿ(ǟfbÀ;Ì
V)ØAÀ<ê?ÉC«P@ Éí
4?þáÁçâÓ?ÛÚ-þ•ò›?²ÞÐZuíB?ÚÂÑ84$@	Î{"¶
¿ïü3ŒõFi?ïþ^‡tÔ¿çQ°''¾¿â?bžÍ¶¿V"ì"q¿ðUNASNone?ïÿá&k€>ñR²Ab>îٔb€ø>ñR²Ae?ïþ"˜»í¿?I¯âaXöY?&ÆtA$?I¯âaXöW?ïÑvVåP‡?€,mã=÷?wDԍW¼b?€,mã=÷~?ïÿJl
æJ?N!9c°†?²~£6ÓJ?N!9c±O4FGL J0642.4+1048?Õÿ…)¡€@{XÑRm‹À9ïL}‡\À;'Z5Ö{¢@‡åÇÅ{ö@F¿Ä§?ɐ]b²?ÖIí{ì
@>)#øÁ@TbCÁö°?ïä©B."Ó¿ßÄøÂôܶ¿é¼O§@¿çòáԛÎ'¿ïÿùSt?ïø#ÝÕ³¦UNASNone?ïaVï<­?¤?äi*Ã?"Õ<âjP?¤?äi*Ä?ëˆÏl V?ÍÍñW`¬?ÁÜÂO¦¥?ÍÍñW`­?ê>ƞK^?­¯ªøO?Çå†Ò‡ ?­¯ªøO?íÐûséB?ŸÆِ±ßÏ?±x'ä`µó?ŸÆِ±ßÎ4FGL J0642.9-6501?Ì"1°ŸfÀ9L[9âyÝÀ:‹¾‰=+À<gñx7@qGÛ
þ@¬ÂPr[?È«k=»¢X?²6ÊA'+i?ãEºßd@Ù¢.¾"`¿àûs¾¾—*¿âº›aÅ¿çvx݌b¤¿ã'eMa²¢¿ïÿ¾&@Üi?Á#%^‰MFUNASNone?ï÷'¦C_Ç?Peº¯Úf?Pú³y@sñ?Peº¯Úo?ïöäJ–?k"ë>ó¦º?R7ÏkØÕÞ?k"ë>ó¦º?ï¸t¢0?€¿ÎnH¹¹?âø×sá?€¿ÎnH¹»?ïÞ²íÊ?`VÚ㪳Ó?p¦‰všýb?`VÚ㪳Ô4FGL J0648.6-3623?ã%'ƒV_ÅÀ07jøœ^pÀ:ÐrûÀ<A5" ¼8@û˜‰y:ÿ@ù—"ÆÔe?ÕGwB¬¢á?Ö~<ЕÚ@Þò"z–@%xÄ¥?ïgF€l÷пã"E	Œ³¿å/Gì'Ü¿ê;ÔÂd"¿á—½¡`¸R¿ïÿþó…õUNASNone?ï‹
·rhó?'";2 ?<'#eÃ+?'";2 ?ï™|*¯'Ò?£ÝÜÀžÍ?‰ õT‹}?£ÝÜÀžÍ?êêÀµT?°Ò'j?†y?ÄTÿ•+â²?°Ò'j?†y?îÙàll0?:lï
ÿ?¢oñù9=?:lï
þ4FGL J0650.2-5144¿ê±4Ýx"aÀ5'	"ãÿïÀ:â$GÝå#À<ž¡ü>ª`@!N
©§-×?øñ¤óið?ҋ‹#ŠÑ?Í5Táä·?û±¾‰=+@†+ëÁ.´?ïúöv'"¿íx¾W¿¿×ÉA|¢¿×Û;Û"zÿ¿Ý;ƒ"…F¿Øƪß<;UNASNone?ïüí"3é?5Dƒr—|'?8–îgp´º?5Dƒr—|?ïúɨjD?c]~±"p?DÛå^Vîå?c]~±"o?ïÆřùÒ?{-âBìX?|3÷é?{-âBìY?ﮈ$Æþ?q7<Šl©Ú?"]öúN@o?q7<Šl©Ú4FGL J0651.9-4330¿ÐZü@'À24GñQçÀ:Ò¢ªºSNÀ<K Ÿ²¸@¶å‹Š7@jUp
?ÖĶv$J?â³7É
û?ýDr‹7×@
M"¿ä|m¾I|¿Ñ!åBq£¿è%–ýÝæÑ¿ïö¶?¯?îœÏä¯A¢¿Ëg!!bÑ1UNASNone?ïÜ~Òïé?`éÈÀT?qÀ–÷9?`éÈÀT?ïøyLå_Ë?wŠ]ŽuF?NÌj€Ò?wŠ]ŽuF?ëuïÅó?ª">Ѷ?ÁŠ(@è3"?ª">Ѷ?ïò›ìIµ?[¸rŸÔ§?ZÈ'l•Áá?[¸rŸÔ«4FGL J0652.8-1855¿è>ö«ÜƒZÀ jÑÐAÌSÀ:¤V¦ÖÀ;¬ƒ•KV@@™vÈß,v@±«Vç?Î3[!8ßÅ?ÇFM^;J?÷b¢Œ‡b_@¯ãËh?ïÛ †ó¥¿äÒ¬9¯N¿äÕK@ÆÔ¿êäÞבL¿ïó¾ýq?•¦í}XUNASNone?ïC¨˜É?ù÷)'—	?—žêìæß{?ù÷)'—
?ï.`'l?ª_×ýÂDë?š3ï½RE?ª_×ýÂDë?éa
Þc@?µ¢¡5Ë?Ê{Ȇs?µ¢¡5Ë?í†NœmÈ-?š¿r§F)?³Í‹'¾¢?š¿r§F(4FGL J0654.0-4658?äp,·…ö+À3
#Ä*fÜÀ;ja©ÊÀ<Y­}|,¡@yåŸ+ª@ù7ªÉm?Ãr(üÎr>¿±€ð«NLê?íçAÃîä@ƒÃvŒÏ1?íVþ–¶¿êŽ|/%‡¿×Jä•@n…¿ìg«ud0+?½ÍË`¢=h¿âŽ9žÝ%`UNASNone?ïï±pè_?`–TRXÒ^?`Næ¡$?`–TRXÒb?ïúh:Òü?jiÝ9úù?F_´¥ƒ?jiÝ9úøþ?ïuÑHEe7?‹û<²9!?'EÖ÷SY/?‹û<²9!?ïì:ì="X?ZlB€Ò†ß?cÅÂ{§j?ZlB€Ò†ß4FGL J0656.5+4218¿·¦äw:Ò@2ÄÓ¿/UXÀ:û
ìQÍRÀ<~܏¸oH@ êÝïßÌ?ýÚy°Æ?ˑ<ÓÅåR?Ƙf?Ïú?üvÕIs™@€ž'&ޑ?痢–'R¿à'ƁY0ô¿³ðýmZ¿Ú7Ûu¼Æ¿æšaÙ¿Ï×æ'öÀUNASNone?ïïZÌ-Ó?]W´bz?`¥3Ò,ú§?]W´b{?ïéÒ·…®õ?'öôaÿœð?f-HzQà?'öôaÿœð?ï·á(Ü­?€	¼°*Z?'µþHÔÅ?€	¼°*Z?îàØÑåeÎ?…Íœk5—K?¡òrá©£!?…Íœk5—L4FGL J0657.4-4658?é‰}ZÌ"À2'¶|(o‹À:ÈÈðŸ:À<›7W…"@Ý)ÆøÍ\?ýËj|uœd?Ì<>Y'?ß<Öàvø°@
¿Þd¤ÅG@Ia}žf]?éù¹à?Óë{#6æÇ¿Ø«€ÁF¿àå½^šÀ¿ïþ°_-âç¿è1ö½aÿUNASNone3FGL J0657.6-4701?äÁ¬ÉI'?Èbp³ÒÝA?×Ü|¦mm²?Èbp³ÒÝA?Û[
ɶsí?ÓÞ¿,m+«?âRy$Æ
?ÓÞ¿,m+«?×oҖAs?¿?†vß-6?äH@´ßG?¿?†vß-6?ÞW·Q쿚?·"VtƒÅ?àÔ$W	 3?·"VtƒÅ4FGL J0658.7+2318¿à9Ò	×4§@'Ñ"D¿À:Ï-˜¿À<eÅööq@&=Kþ@غ@Ù$?¸5%¦­©¿'µÜïB?·/ù‰@ѾÎ]?îÝ)4­¿àø»Ó€E5¿çË¿m"¬¿äsšA	_¥¿ãbá@øÔ¿Ò&c«KžUNASNone3FGL J0658.8+2318?ïñ~å%?W ¸ãA(À?]5õݵ!?W ¸ãA(Ê?ïû€‡á'I?fëыƭ?AýàyöÜ\?fëыƭ?ïÜ"' N?s ÂïÔ?qñµ¶ïØö?s ÂïÒ?ïò,°Æ?FÖh¡§?[٧Ԟtê?FÖh¡§4FGL J0700.2-5118¿éI×U¶ÐÀ3‰æÿ}úÀ:ü`8NûçÀ< !¥l5³@—€Ã^äè@óû¶Å$?ÈW2ÁÉ8™?ºäù}º–?ð] ½é¨?õs˜Ôw¼?ïû¿ß(™ý¿àCòÖKҿҁ~ƒ=¸¿äÐeÁ•a¿ïÝUE¬²{?îíŽ]ü4™UNASNone?ïïJ1o±?dÞ›‰‡?`µÎNða?dÞ›‰"?îé<ù>ìá?°ceb_·3?¡l0l1ã?°ceb_·3?î觝D	?"ô"RŽ…B?¡u†+¿n²?"ô"RŽ…A?ìäß:ï}æ?¤É¥
'‹?¸Ù("Ñ?¤É¥
'Š4FGL J0700.4-4308¿ÞVœëV"À0¤a¶Ô=À:ž;¼n°¸À<AäMòÒ@ý¦kd@8—Ü*7â?ÄÆFuÛ#}?™|cÓ¹ü?ÐԁLá@©zJP?×,B®{S¿åV«€'¿îÆ!·à¬¿¢	_$RÅ ¿ïÿÿ" 5•?ïó@oܲUNASNone?ï𘡮!?c^_—`·?_Êμ£¿Á?c^_—`¶?ïˆ¼?|öòÄF:K?`tjpwBX?|öòÄF:K?ï˜êZ|?"h¿ñ3?‰Åi|àøš?"h¿ñ2?ïò¿(.½?S/ùàr?Z¯¢"üy?S/ùàs4FGL J0700.6+3558?é=Ž@1Cð#éêÀ:¾í¥Šh¤À<…˜f"³@þBƒ2O?ÿ'
;Qå¦?ËB%ŠÌ?Ø#ïÞʦ,@
9'N"¢Â?ýNÀ'"ß?ì'JSá)¿Ðè=µ¿ÜÞÝÛèɃ¿å¬•õ *­¿í`Ÿb0vÀ¿ïþ~á•›UNASNone3FGL J0700.6+3557?ä$Ahÿ²?ÉM•â•Ég?×·}û.œ?ÉM•â•Ég?Ý?Ê/¡‹?ÒNÓ(ø?á`è/:?ÒNÓ(ø?ágØnýG?¼òÌî•Í?Ý0O#îs?¼òÌî•Ï?àB«µŸË?²V©3iì9?ßz©Þ"Àh?²V©3iì94FGL J0700.8+1551?Ð<Ó¬·»{@"^ËtÝønÀ:ÕZ±&~À<u˕•(@›Ãl{Ô7?û6KÄúp?ÓoI#Šs·?ܪù=n˜@Õe!ÂÈg?ýiÀÆY@8?ïøc‰<TD¿Õ×u1ÛD_¿£âï#
÷¿Ümz÷÷ž¿èƒÜ=®l¿ïÿËÝcßUNASNone?:iàžÄ?‹‰SAL†h?€Ùe‡ØO#?‹‰SAL†g?ê(.YÙÄ?ËN±P^͞?Ç_Fš˜ò?ËN±P^͞?íX¤?¥BŒ;"÷?·Õ?OÒÝ?¥BŒ;"÷?æÁ½½þë½?®ï‹äbnÌ?Ò|""(…?®ï‹äbnÍ4FGL J0701.3-0403¿ã셽½Æ‹?ÕÏæݚ$"À9dYbqå À;BöÜjς@aR½è@Rr†/YŠ?Æ-¡º$?Ͳt†åŒâ@%ÏÅ¥'?ûPü#ý`>?îèŒEô?Ð)ú¥M,¿ênar
ßW¿è"»ìª¸¦¿ïý ‡_r¿àÕ,ß?–UNASNone?Ôô>AÊÓ?кdðÔ?å÷àß—?кdðÔ?ÚøøwŽ3?Öêb"¿\?âÿƒÄ8æ?Öêb"¿\?ÜáŽ/ªÒ?·çëOi
?á8è*–¹?·çëOi
?ÉáÕÔ`â?¬>Î;þ©3?释ŠçÿH?¬>Î;þ©34FGL J0701.5-2842?Ü¢;á4ÚÀ%GOøe×ËÀ:ûІ•°×À<CgUy¯@lþáòο@Y™~Á¦ÿ?É<Õ"oß¿›'Z¹gž?Òo_Éî@×~I1!`?ïݬþüõ?£`,¡¯ÎË¿ê§ýuDØ¿âTÁ"tŸ¿Ò‰À¾Kª£¿âª†7"ëUNASNone?ïí¯y	Ÿ–?ab¾àýª/?bP†ö`jZ?ab¾àýª.?ïþ:Æ⏨?PÚ4¬ž"d?,S'×{?PÚ4¬ž"f?ï dœÿà–?…#Õb}s?‡æØÀÚÌ?…#Õb}u?ïô·Ò`ľ?E°‰Þ¢x?V[>vƒÇ?E°‰Þ¢‰4FGL J0704.3-4829?Ô oþ*À1ô$¢v·íÀ:º¶â¼yÀ<V "oeé@ ]¾!8_?ÿoÕ`EK?Ìvô©	Ï?¶vS€ÕS?ìki¥¶Ž@ëuró½|¿ïñ±ôr{?ï÷á]¨|¶¿çi2(q8R¿Ò±K¼ìÚß¿åžbP2¿ådi×4.ÜUNASNone3FGL J0704.3-4828?ïÿ"V"Så?¹`ߢ´?ê[+y?¹`ߢ§?ïývnPÝ¢?Uëjf€¶?4Lyñù?Uëjf€²?ïóµ(υo?\7ke\dº?X•®`õ"·?\7ke\dÌ?ïé6¡Ë³$?YØ¢Ýх?fÉ^4LÛß?YØ¢ÝÑ}4FGL J0705.8-0004?á$÷êfL@	\[cÓåÀ:"Ö¼À;¾7¹ª±@¥pŠí@¹÷<âß^?ÊàÓnu)?ÕYâµí7@ñžBuÆ?ü¹¼yÃep?²Áýäê%?ï\ÂMÂÖ¿âQ%!!¸·¿éè¢ì(²§¿ïì7Ì'ã?îi,êCÖUNASNone3FGL J0705.7-0006?ÒxvTg¿¿?ÇÝJ_=ò?æÃÄÕÌ !?ÇÝJ_=ò?ØéDz&Ï?Ԣκ]ð²?ã‹&õl™?Ԣκ]ð²?Û´™g|‹Á?·øp<´‡´?â%³LAº?·øp<´‡µ?Ó˲4Öß?»{©—K?æ|¦å"?»{©—L4FGL J0708.6+1747¿äÎy'èd@'k͚R&>À:íÚü:x¢À<c;8»2@ ‹34à²]?þ{®—WŸú?Ð6[œ2ü?¶2ðÞ¤æ?ꖉ1+?ÿB¥Áðü¿îÉÔž›·?ïý¨6ëN˜¿å-ë?ÿtj¿àȖg"N¿×R[ø#h¿åû®Í…/UNASNone3FGL J0708.7+1747?ïý
Hoü?3Ð@~È£?7•¼€Í?3Ð@~ȗ?ïï5K_•¿?~Pð8Ìé?`Ê´ j@??~Pð8Ìé
?ïåã±ëhm?l°yh?jN—'Œ?l°yhþ?ïŒÝ!0e ?{O#A×,A?ŒÈ·³æ—â?{O#A×,C4FGL J0709.1-1034c¿Ñjfõ:R ¿íKÒ»úÀ9!ÌzdJÀ;1œ_F·t@üx±—'-@ÁåGíÕ? y‡«ZŒ?ÓÊ89W@¦ÜG©ã?þ0n&nª¿É¢ãj_D¿ÞÒý¾\G¿èQÒ?ÓT¦¿é°‡ÿ=¿ëoc/zA¿ïý…1,ȶUNASNone$?§'C‹VÉ ?¨Oê'"?ÇJ"f?¨Oê'"?¿l¤ì4‡í?ÈÖ勠1‰?ìkbyo?ÈÖ勠1‰?Ê¿,c?±è8ë~?éP?;>ôç?±è8ë~?–³¤={š*?}R퇶|?ïJbÞ#/?}R퇶|4FGL J0712.0-6431?Þ Ì‰$ÄÀ6*¦óõ/ÂÀ;'24/²uÀ=ï4Ö¡b@§!,JŒ?ý8ø¤ÁëÈ?ÑUØInß?çï~U@Jâ|az?ùÜ÷&èw"¿îªi?ߓú?Ó߁w^¿È*è7¿ãÆ}'s¿ïÿ¤Á	?¨~¡½÷¿6UNASNone3FGL J0712.2-6436?Њxòˆº?Ŗ`;‰§C?çóºÃ†»¤?Ŗ`;‰§C?Ó=TÖ³¥?ÓùÌè©07?æaU"¦-y?ÓùÌè©07?ÄNa½†9Ç?±`J??êìgžq?±`J??Ɩ?Úë-?¯–fXzÂ?êZp9‰E5?¯–fXzÂ4FGL J0712.8-5637¿íöÔBŬÀ3"µþT.UÀ:¢P0™û¿À<bg.'Å@ôê†ñ÷)@"dUêî ?ËHhbj?Öq"'›@x—Ü*7â?ÿ5Œu?æâ"Ÿg9¿Â'N¹Ìiû¿èϕÔèû¿ëf YžØ¿Û<-'ÅË¿ïþæZ<ŒxUNASNone?í`çÉ?¶a°*ØB?·4üÇy½?¶a°*ØB?ív2ÏBH½?½'h¥Ü…Î?´Ni…íº?½'h¥Ü…Ï?éU@okm?´ýÇa;fo?ʪþCúRJ?´ýÇa;fo?ë?cÁܒs?­‰ìmLNj?Ãpø¶6?­‰ìmLNj4FGL J0713.5-2555?ﱶ6p+À Â	$lÀ:`öqÀ;ôó±³l@"®R
hô@éu½~â?ÂC| 7?•g'ߐô¯?ÖÑá^ª/i?ý¼&1$4?ïa‹€|<<¿Þà¾FL@¿è´÷Ãñ[ø¿èû9Ç¡ë¿Ð±©ûçl‹¿æD˜5kUNASNone?ïÞZ¾Î~Ã?iˆ&cØO?pÒ ˜ÀŸ3?iˆ&cØN?ïèYZœØb?'ùJê¬Ëº?g¦¥c'V?'ùJê¬Ëº?ï/µi/?ŽÚ,dü}‹?š	^üÚ
?ŽÚ,dü}‡?ï"ãí½J?x+9d½³?ŠÇ"­u?x+9d½±4FGL J0713.8-4820c¿Âé@î¶À0q+àŠðÀ:Ä©°ãÀ<G#çÆM@«<Û}"«@âÑk—þ?ÉâxÉhi?™OSǟ³±?Ñ&±dç`L?ý¨Tßd¿ÖX‹ýy½Ü¿ãCÿ~zÚ<¿ékEÞ±{¹¿Ûý¥|üªá¿êöÁBU&¿ïþ:bÒ]0UNASNone ?ïèÞm"ï?e‰5³Òÿ?g!'lâŽ?e‰5³Ó?ïϏ–ܲ¨?'C»'?x84'¦¬?'C»'?eKp¤?"†Á#ÿ¬?‰—f­#Öé?"†Á#ÿ®?ﮒ‹Ý©?p£¡ï' »?"[]ȕ¤?p£¡ï' ½4FGL J0715.7-1128?î˜I,n¿…?´ÿ¾'ÜÈÀ9¼÷~0ˆÀ;`Πâc7@o!c'Å@¢Ž…i`í?Î7^¦~"j?Ú°km6d@@º°k?ꏳ`Xôþ¿Ü*«Ú佄¿¹ž+࿯¿èðCÊZ+Æ¿êN›n…êLžsóí£¿ç+ áCUNASNone?Û´ÈD&j?×óµžYs?âw¥›ÝìË?×óµžYs?Ñ0sg£]?Õ©UV™?çgñFL.R?Õ©UV™?Ñ%-Ø:Ë?²îRHŽV?çwmiâ›?²îRHŽW?†×ÙKåéŸ?qÍD¨{?鸞šÐhY?qÍD¨{4FGL J0716.0-0826¿ïQ'bî"8?ù<¼~ ïÏÀ:$OTÑélÀ;¬ÓW*‰A@ç|\@?"Àh¡?Ð(Zý|˜?Ô)ù"Á ?ùb.þñG?ñrZ5*¯+?´Äúâ‰Í¿Óãº¥¿èq'>3Av¿é¢á ÁÁ¿ïøìˆ3@?ïÂpóˆ"yUNASNone?ë½€™ˆ'?Ä)m¬èÿ?Ãñ	ý™ßf?Ä)m¬èÿ?äYÚ}U¹-?×.?=—©Þ?×LKT¦?×.?=—©Þ?âñHEp?·¥6lHÉà?ÛÀouÃ?·¥6lHÉà?ÒíAÇfD?º‹Æ2¨?æ‰_LÞ?º‹Æ2¨4FGL J0718.8-5004¿êï{¯Œ¯ˆÀ0Z\å´$_À:͇
JܝÀ<…f?Ð@³â@0Ö­3ª?Ëq}Ü#×Ì?Ú~FïƒÜ@¬>/æx@ ¸=s¨ï?ï›ÞÒê¿ÒOZ±&~¿ÜŽèÑQ­¿äÞ!ž`RÑ¿éO"¡2O¿ðUNASNone3FGL J0718.9-5004?剽Ǟú?È/9'±!°?Ôíø"pÂ?È/9'±!¯?áš~êVû?Ó	•È3­_?ÜË+õR
?Ó	•È3­_?ÜÃUJ?¾pðoÍ	:?áý{ÕuÛ?¾pðoÍ	:?á)šª.µŠ?³ ¹'<?ݬʫ¢"ì?³ ¹';4FGL J0722.4-2650?³\Üp1JKÀ¬	Þ¦%À:ƒsñidHÀ<D)ÿ®@\ó4ëo$?ÿ:¤þQª?Ð=;"G?á%K~ƒ"ž@aL¾´?þšBѶÁs¿ëqA@'m¿Ú‹2äôQ¿Ï4`¯Ã'¿åËDÂ&ք¿ïý¨¢K?¦«Qý΢eUNASNone3FGL J0722.2-2648?äÉ[=dî?ɕQs^¥ï?ÖmIم6'?ɕQs^¥ï?ætåDÀmV?Ò0.NSE@?Ó5v%R?Ò0.NSE@?Ú1MŸx©™?½}Ã"TÀ?âçY0C«3?½}Ã"T¿?âÂ'/…?·`‰fóÆ?Ú{± ßö÷?·`‰fóÆ4FGL J0722.7-2309c¿ÆëB·À:og—À9šñÎäÕÀ;LzÜ?0—@Cÿ‰7¢@y͛ÿ¥g?Ê»y'¾?ÓE‡~d	@	êºp©¶?üXùÁL'?Uª×¿å3éèwM¿èՉÕwõ¿ì;C½Äò
¿ð?ðUNASNone ?ìÐ3f›±?¼ÖçézïÒ?¹~dË#z{?¼ÖçézïÑ?âE?œ´L?ÕÔ©sf8d?Ûu€Æ—Õh?ÕÔ©sf8d?ऽ}S¹?·òß"š%?޷ЅX?·òß"š%?Æid9³o'?³Ší®y3?êe¦ñ"$5?³Ší®y34FGL J0723.1-3048?ØY=iw¦HÀp®SeâÀ:¬ä_‰PÀ<<v`¯m@@ÅIìˆ)@NŽ£œQÛ?À÷5Á'쯿˜šŸ˜·?Ü´O'…€?÷Q•"&h?î"gñ€á<¿ç[}Õ¿å÷ù1~'¿çŒþ«—¿Ú¡ûÁVÍ¿³+ooyŠ…UNASNone?ïðOªï|á?Z¯'íêÊ?_`ª!>4?Z¯'íêÊ?ïÍÓ¦'^ç?=kq¨ ?y,¶Ð‹þ?=kq¨?ï¼Æõ"™å?~ôàèܝ?€ÎBžÙ†{?~ôàèܛ?ï(Ÿì÷|d?…RÏzõäí?šìasd?…RÏzõäí4FGL J0724.8+3016?½ìòÑ@3öuy(àÊÀ;±™]3·½À<½`µL}‡@#nxY$È?ùÝ5µÄr‹?Ƕ÷xr¥¿¨ócå$?âEy¡¬'@šŽË·¿ïÿDÿ8"×?ïÿï0l¯¿æôpŸû2'¿Ñüf£".~¿ê•ïUÑ?áºæ ³iNUNASNone?ïÿ8Ui*Ç?!fçîVv?õRÚ§R?!fçîVi?ï÷'Ñò?'–ô|eП?Q±Íð\×?'–ô|eП?ïªôRK?ƒ¬¸uՖ¤?…Bëm¿f?ƒ¬¸uՖ¤?ïêÂ÷?e¢á\ލ$?e=ÿà^?e¢á\ލ#4FGL J0725.3-2550c?ã øBÀ»À†¤û¨'À9Íí'?2EÀ;c¡®;N@-8œ(À@Åôÿý²?æhàÿ‰¸{?äužö$à@
-«Þ7@È{"ZÃ?_î}!¿á¼üJÈü¿èÛrLM¶l¿ïün{Þ¿èÁÞ\AIv?хõB6Ü5UNASNone ?ípQoz…)?ÁWÆ*éø–?´}t"+Ö»?ÁWÆ*éø–?â=)k·-?Õ¾5(Ìkø?Û݅­('¦?Õ¾5(Ìkø?â²(A"?µeäW"ˆÖ?ڛ¯}»Çã?µeäW"ˆÖ?Ë}{}ðl¿?½Î_"v?é ¡ ƒäÑ?½Î_"w4FGL J0725.6-5008¿Ýô•Â~®DÀ.À'ÏR¹
À;/ìVÕÐÀ<"ՐÀ­@ ÃÉñ%F¶?ÞW> YQ?Þ%œSÞ$?ï‡ÁàŠ™Ì?ýC·zU0´@-'U°5½?éQS¿Å¨@?áµVÄ1ó˜¿ëh"ÞÒ2è¿Â2ÏJ«tã¿ÍGöµÿV¿ðUNASNone3FGL J0725.4-5007?ïÁY¨ƾ?€;r:1¶Ü?S+òœ b?€;r:1¶Ü?ïèï—s=Ç?›G~Ö!/ñ?ghŒÂ9y?›G~Ö!/ò?ï+2Ö+°?'ˍx	Ž?šœ9¥:‰ô?'ˍx	Ž?ﶉ§#¿?}ɑ'*"?']»V7??}ɑ'*$4FGL J0725.7-0549¿á`Ґã»@¼ŒÖ<¸À:$ÕϪ͟À<'¤ýzê'@ ·E¼wÀ?ü.;—…Ã#?Äãâ'§ä¶?Ã"?Zˆâ'@üäŒØ@s	¶Z?æÝÿŸ²ãB?í€FacGM?Öå±àHþ¿ÛOȶ«¿ÜìØ:¿¯¿äJè0-UNASNone3FGL J0725.7-0550?ïÛ$µ—?s…«0?rmú%y´»?s…«0Ž?ïÚDÓ§P?'U<Bé-9?rô]–,Wð?'U<Bé-8?ï³3
җ!?…ríŒÇÞ?ƒ3<‹Z7Ÿ?…ríŒÇÝ?ï?撸º?†Ú»Æòš´?˜-¨þh¼?†Ú»Æòš´4FGL J0731.0+6607?å°e>Å@<ž"šVWûÀ;	µólÀ<°5ŽWF8@ß\>oQr@N˜™¿YG?Ï^ç–ýˆ?Ë
ïWúh?ûѽ¥è@$ÃÆ=ç?Õâø]I\??ì'©
Oå¿ß§ñ¶'!%¿àt`YÜë(¿ïÂXúìñ?ë6ElÛNUNASNone?ì¨é›…5?³F"Á"?º¸³#×ö\?³F"Á!?îcþ¡(›?·ÎfùE?¨	ÀívZ?·ÎfùE?ìfÿ®"ßâ?¥yRNE‰u?¼È‹Yç?¥yRNE‰u?ìšEU;²F?¨­<4?»-ÕV"mÓ?¨­<34FGL J0731.5-1910c¿ÚÌ0W±ñ6¿È*VÀ¬'À9vf}ãZ®À;$(U{]@àšF<Ð@@sÀÁü?Ð`ÏM°Œû?Û¹1Å{@Ÿ€Á[ƒ@oå¤ßóÆ?´¬˜¿â·Í⠜¿éHL՛¨h¿ìÃ+c[¿ïè¶!å'ü?ï£êUsÐUNASNone3FGL J0731.7-1914c!?ÙÓYǃU?ÎÑI¼®s3?ãqS>V?ÎÑI¼®s3?âšúcŒ™¯?Ö<B`,ä?ÚÊ8æÌ¢?Ö<B`,ä?ݱïÅ?¶£«Xí¨?á}'s}?¶£«Xí§?ØÓÅgϊ?¼ò¡ÆVù?ã–L:ò?¼ò¡ÆVù4FGL J0734.3-4448?ïìY~·À'ƒÌòŒyöÀ;ÔÈ("À<bZ¬ôÀ1@ Z¥@ð@>GÜ7£Û?ÃÍí^<Ì9¿Ÿ\1%´;ÿ?ÝC]÷)?ÿÈ¥Ó¹¥ÿ¿¼ șڿá \a)惿éQÓÂ_`Ž¿ÞÀúôÓQ¿á]Õh|Á¿Ö…Ôàík(UNASNone?ïúT]vp‹?AŠ´
C)Ž?F®Š&=Õç?AŠ´
C)‡?ïó½éK§`?tc÷qƒ"b?X"-h±>Ó?tc÷qƒ"b?ïëI Zb?lo?"û˜Q?d¶_¥÷?lo?"û˜H?ïÑo4›¹*?dñµU¬Ì=?wHe²#jþ?dñµU¬Ì<4FGL J0736.9-3231¿ÅÆ;>ÀL™Â´EÀ9RyaíÎÀ;'¦éä4È@ˏ¼ÈÉ@$§š
\à?ºürùO7?ÕÒýhv@¦¢‹°£@—Ž§x*?ïÿñ_{'¿Ú;ô¢Ô«¾¿åÊZâN¿+¿ê÷']gå¿ïÿíPÐÓ?ïñÂjÉ"UNASNone3FGL J0737.2-3233?ÒµùJ[à?ÉZgý­á?æ¥ZýR?ÉZgý­á?ÈZª9˜_–?ÍÜ"ÃûÆ?ééUq™è?ÍÜ"ÃûÆ?Èz+ª?°
·¥zs?éÄ¡u?°
·¥zr?Ä«‡R$"?±G´¶üÒ?êÕ+z¶Û?±G´¶üÒ4FGL J0737.4+6535?ïH«Ú	¼µ@=@W:yx'À;TûwCÀ<Û:aû›@ Ÿï 3Ò@Ðh˜oÍî?¾¥õÝè(¿±Œ,ž™ˆ¨?ôn$ É8Ä@‡ó]ZN*?ïì³I¬¿ÒZž\!¿æø'}sHL¿á˜çBsB¿àØÏo>|=¿Öј
¨_/UNASNone?ïþœLÔÛ!?!àwS#í?&;2²Møž?!àwS#ò?ïýä0Bl?G­s"&ÿ	?0߆}ì¢Ù?G­s"&ÿ?ïöIT
Ð?`'.åKôx?SmWê_Âh?`'.åKôr?ïéWÊtJ?Sזì'h?f¨5‹¶Ë?Sזì'l4FGL J0737.7-8047¿æ®î¼¹À8îÉâ6Á]À;mðwÌÀÀ<®rØœ@"E…sª?ûêՖŸê?˹®øP‰/? 33"'K?֓7_'·¨@–Æ4WK¿ïéZ¢
¢?ïödá+(£?êàöðŒÅv¿ßýS]?á¿ËA×e×ö!¿ä?y'"UNASNone?ïÿk^ö‰­?–úï7–l?"!.ÊQD?–úï7–™?ïþ~óžÊ½?JŸ_y'V?(ÆT/o?JŸ_y'V?ï퐕j¼Ð?e³
Ò'¼?boj•C0'?e³
Ò'´?ïù,﯆ô?B!ÈF¬§†?KLAAä1ˆ?B!ÈF¬§'4FGL J0738.6+1311?ÛW5)ìºÊ@0TC^úa[À:¡1¦¿óÀ<TÇ$íS@wð¶6y@È7 þ}I?ÀŸ9Q´~¿šÛ"CwÆ?Ô6߇Ï@¸¹jyN¿¥´)gØV¿éyô'ô;§¿ç)GŒ†‹ ¿ëËì't¹æ¿¹` Ò¿ç†lªMFUNASNone3FGL J0739.8+1312?ïúáÂlÑm?FŒX|öåç?DxöLºQ#?FŒX|öåã?ïýUÜS2?Xw'#ôž?5Qfl:?Xw'#ô?ïà`keƒ¦?rM%…<I?oŸ"š|Y?rM%…<H?ïý7–°¢?*˜xÝi<l?6GSJzñ‰?*˜xÝi<)4FGL J0739.6-4530?áŸF]­=,À&~gµñ¾õÀ:€ÄK"À<ùqp…¤@üoò2b@ùI¥e·?Ж@.l?Ê"hܸ?û‹Jì\t?ð<x{í¿èIg–Øõ¿ßܔÀìĺ¿æ¢þ)q¿äç½~{0"¿ïÿ}ž¼C=¿ïÿ·¥ôïUNASNone?ï1q¦¸7Q?£u7—s?™ÑË(ùÎ?£u7—s?ì2Í®Eb?ÆàÿÎí?¾i'×$ô?ÆàÿÎí?é!g=N‹?´ï/¿š?ËzcÓ
ÅÔ?´ï/¿š?â"ë«©9è?¸',œŸ±y?ÚÖ(¨­Œ1?¸',œŸ±y4FGL J0741.0-5226?ٟ
Š—çÀ,Xépq'#À;wï‡â·ñÀ<Œ¬&dØ@#E†•…ã¯?üCïÉQJ?Èùƒ<Ù¥¿±P;ל‰Ž?êÀSAÆsí@¸(Üî'¿ÌH…ªÏL¿ï-¸À%t"¿ÔM›iR¿ßWçÝõ>0¿åÃcÍ.ò\?´å€ÝNêUNASNone3FGL J0740.6-5230?ïÿµUÁ>û7à¥å¾À?¼*¼Ť>û7à¥å¼à?ïþ€U2x¤?G±á±Ó…?'ú¬ØuÉ??G±á±Ó…?ïú5âaÑ?^¯H·íøž?G(vx»È'?^¯H·íø¢?ïúö
à^?Dä)&xº?GŒ'Ô~‡ä?Dä)&x©4FGL J0743.2+4034¿ïm©È¾@:Yæ%cgÀ:ÎÓU}
À<~Güó@ÙJ¡!@|âąÖn?ʔ]Úü_?¸hšÉŽò?Ù‰@¢ŸÒå?íáH2ž¹¿ëzá³
Þæ¿î
# îø¿×,RÙÁ§Ö¿ïÿT©¥€X?ïÝe¡D‰UNASNone?ïòÒñmüé?—Ÿkú2k?ZZ$,á?—Ÿkú2k?9¦Ü?¨Ú#ƒäø?Q1¹VHü?¨Ú#ƒäø?ï"ä;?°?"£œü끉?‹û10ý?"£œü끊?ïÊ»¢vŸ7?x…d Á?z¢.Ä°dÅ?x…d Á4FGL J0744.4-1403?â^íðZ\õ@‹"ÞQZÀ:Qo­7PÀ;å‰bÙ@̀;¤›Ö@ÖwÁ½o?А^\¶#?×>š?‡@T¯ÕEAS?ôBñ—1Š?ï³ÃçJýT¿æÕ `]7é¿éº øžï¿ëÇC‹p+¿ã%áæåR¿ïÿÕ¾
iUNASNone?ìËNWid?ÁÍ­0ÌN=?¹¥-D´Þ?ÁÍ­0ÌN=?áïÙ¬?q«?Õï¾Z·Ò?Ü L§ª?Õï¾Z·Ò?å)$×Áq?»Yj®â©?Õ­ý¶P}?»Yj®â¨?Ò8Hxjð?º-·#¡I‹?æãþÛÃʈ?º-·#¡I‹4FGL J0744.9-4028¿ï×ÒtîƒÀþô›»³À:mµWeA£À<f
w"@š—ƒê°¸?ü˺bfý?ɪ`;Tþ?ãÄZ7ƒúÌ@ßbц@X—²Ž³?ïz͑êØ¿Òê?yg ?ÂâÙ(¦¿äÆhÏÍ2M¿ëFz£4M¿àƒ ˆ÷
UNASNone3FGL J0744.8-4028?¯—C,j#å?´lDÀ·mC?î‹Í9]Â?´lDÀ·mC?Ñí†w°^Ê?Ò/Õ<xJõ?ç	<Ä'Л?Ò/Õ<xJõ?ªŸ:‹R"f?›ç2}bÒÎ?îVWJÝÙ?›ç2}bÒÏ?ÒÛ8‹èÃ?²"?ÅtC
?æ'cº9ž?²"?ÅtC
4FGL J0746.5-4113¿ã}É5íFžÀ 6‰Å!ÞÀ:«°ÿç¬À<IP«éþ@8ñÁ"õx@›²ãízÂ?ÊÄ3êé?µ•þk?ì«Ð¾Hûq@^ðTf^¯?ïþÖ~z¿ì@9
ãˆÑ¿ØOr"¿ßó«z=¿ç›#§¤õ¿âà¥Ç¥EŸUNASNone?ïû0¿¢£?OàPqãÊã?C=uqÂP?OàPqãÊç?ïü"ä5©?UÃû{Ü7?;ßPÞR¸ð?UÃû{Ü:?ï¶°Ê 3ß?"bŒ€Ât'?'SÍwó?"bŒ€Ât?﮼&ÎaÓ?kkrÂyO?"PöLg‹<?kkrÂyL4FGL J0747.2-0736?ïÿíƒ1 2@!…–À:Õ¹Nè›À<MÓÔ(
á@ Œ-·c?ÿÚÇ犾5?ÏÌçå,0?ªå Å®‡?à(È
Æ, @Rn6êM¿Ùù–#ÃS§?×ƺCÞ&;¿á'àb*íi¿ÙEÉ7ìÖX¿çÂb¿¤?h50ìåy UNASNone3FGL J0747.4-0734?ïúƒnŒž­?F·º«7b?EòEͅI?F·º«7U?ïò¶ºR?~+·æ?Zä"è‹ZÃ?~+·æ?ïÒè'^?yÏ̍ìß?v‹À>ñз?yÏ̍ìà?ï­ûÇÕð³?ræ×ßÛ0l?"
ƒÓd?ræ×ßÛ0k4FGL J0749.8-4420?å±/žåtÀ"3󾩛À;9
£3vÀ<µ"6Æf@©ûv®] @RB<»r1?Ò娛•\?äÅýƒxñ@`ÔV.?òasÝó:Ë¿à†øaûó?UAª33¢ß¿»»Ñ«Xß¿è9']e5å¿ëUÛN¿ïÿýawUNASNone?ä"(´ÅÀ´?ÊEà-´lØ?Ö×®–t~™?ÊEà-´lØ?Ü7£Rj³?×~ªâvì[?áä.Vʸ&?×~ªâvì[?á¥R–4ù?»®­s(Sý?ܵZӖä?»®­s(Sþ?´ÆŽëUú?˜lw[_??íg.?B•A?˜lw[_?4FGL J0750.0+7140?âff˜N–@>>A€ÓÏöÀ;'u¸êÀ<^£ƒ'gM@ia ƒî@™æáK	?ÂZ	‹Å¿Á0'B]¼?ð֑§\л@QPiÏÒ¿æ{¼n°·Ã¿çýՃT´¿éØ·¡Â]¿ä´>Kë¿ïüž…¿ïï,"¹ºUNASNone?ïíz4õ…õ?nN™>l•?b…Ë
zƒ?nN™>l'?ï=À/º?¬û×\=	?˜Gÿzè°?¬û×\=	?ï¤fl1
?"ǝ²ÿU?†ædó =œ?"ǝ²ÿU?ïPØÚîC?…ùeHÞ³|?•ää¢7œt?…ùeHÞ³|4FGL J0750.5-7519?¸ti"ߨÐÀ6ŽØ
±À;!n
#ÔñÀ<wñ8¼ßð@–'âòþæ@«Âßä?ÓʤzHF?ÛÞ¨éϒ@}€Ú…ó@Œ T‰D7¿ïÿR@>´q?ïû¾½?'?ì"}Š¿èîê.¤¿á‰ ]9–¿ïüö@
·#UNASNone?ïæ¥öple?jü&@ߤ?iZ	"š¦?jü&@ߦ?ïí:°.Œç?"ÒgK]	?bÅOÑsî?"ÒgK]	?îX9Ùv³? hN= ö?¯|bh"Ë? hN= õ?îÄzjˆúB?"ÛBéÜO?£¸YWp[ì?"ÛBéÜO4FGL J0752.0-2931?禘پ…ˆ¿ômY4N¼&À:¼&Œ[ÃÀ;èH÷À–^@]6fïM@]<9Aj?͐½'h?æêúêíID@^Íñ?ø~…—<¿Øy|ӆ¿µjF€þÿ5¿àùI—ù†i¿ë÷2ú(P¿ð?ðUNASNone?£çN¨¬?¬ÏZ^Í6?îϞ±‹u?¬ÏZ^Í6?ÌRÖ1Â÷4?Òî"á—y?èëJsB3?Òî"á—y?ºä#>O¼+?©k¥ä340?ì£{˜6z?©k¥ä340?•Hbg¼$L?‡tßTIñ$?ïU¼ìÂÝ?‡tßTIñ$4FGL J0753.1-2624c¿Ï€¸Mµ
?á!l—¥À:ŸËz½5€À;÷ÏdVÁ®@ùáxÖU@1ìVuX?؀ÌÄjÁ?îܘQšýG@4' ÷@f"ÄB¿ïÿñò÷?ïÿ@Aä{ë¿â5¯^ý¼Y¿íLE¾P2G¿ïÿýaw¿‹4J_t¯ªUNASNone$?ÛÛD;&¨?ÑþOÄKLI?â]öbl¬?ÑþOÄKLI?Џl>ºS?ӆ¨[Ó½?ç¸Ià¢òV?ӆ¨[Ó½?؎½%ŽÕ™?¸7Í$Àî$?㸡m8•3?¸7Í$Àî$?¼ß"g‹—©?¥Ï~­¦ˆ?ìds?¥Ï~­¦‡4FGL J0754.9-3953¿ë8'LRKÀ?Ë~3ÓÀ:¢rúÉÀ<ÄxCÞ|"@Ž}á,U@?Qi›?ÌEú
G¬'?ïþ¡€Ã´Ë@öÇê弈@WzK˅z¿ïÿú@ùDz?ïþ¯¾3G?æiªK¿Û©q="ðÀ¿ð?íáŸËŒÜUNASNone?¯}¦¼<þv?¿¶Á¨ª©õ?î%"<0?¿¶Á¨ª©õ?¤Ê7ޖR1?¶6æmt?î³\'šÝ?¶6æmt?ÄéFŸÚô?¬øÛkP•Ç?êÅ®X	}Ã?¬øÛkP•Ç?¨ȁF?t|TNš'?ïÀ¯Änýt?t|TNš'4FGL J0755.6+1855?Ð%4A ¦@6_ºº{'qÀ;]K´3xÓÀ<¡ÊVÐÇ-@´¦M@"Åyò4e?ОÖd¦à?yT¿"~ÕÕ?°¥ô›ÈÈÜ@~ù ?ïíL~Þ­J¿Þÿ<÷S½¿é­Wâ1»¿»uøÀ·¼¿äd¶Ê,¿ðUNASNone?ïþÕh2‡?)ž©y-§?"®)|גÔ?)ž©y-y?ïþi}`¡w?FšqÐS#$?)h)õè=?FšqÐS#(?ïæªÊÉö?qì³](?iU56	üY?qì³](?ïùæ{Ð?8ÚÏ¥€Éª?K¼g'¾Ï?8ÚÏ¥€É—4FGL J0755.9-0515?àêÏ´–lq@''´·,RÀ:‹kÙlîÀ<³'àÚ@O—íÇï@ðù'7}E?¿µ2&mÒì?¨VL_KŒh?ãmjñ¢?ôäŠ$[ª¿Ïl?XÛci¿ê-Ôï°ýc¿ët·AË&"¿äü¦¯+Ò¿ïôèà(Ê$¿à†HNMjíUNASNone?ï^h¹=? ]K–qg?"<ÒèÜxJ? ]K–qg?ê–Z!õs?Íuí-PÌ?Ŧ——x*5?Íuí-PÌ?î2̀ðý? ÕZ2!N?®œÓ'ðð*? ÕZ2!N?ên	T¿£?²šªÉäê?ÆGÚ­‰t?²šªÉäê4FGL J0757.9+7304¿ì_)¡À#@>¯½¯ljÀ;Ï1_œÉÀ='òH‡XN@ šj$"?ûÁý¶y¤1?Ôp†yÇ?Îø" 5ª‡?÷*ÑJ
M@°sAI?혬3Ð%¿êVg€AÙ¿¿Ñ
7öçRŠ¿àëL4"†¿Ñ`Îvðø%¿ïÿî,˜å?UNASNone?ïú"¤œº?N#9Ø
hÔ?Guméû?N#9Ø
h¿?ïýREÖÉ?S-Wáé?4mÑI´¸?S-Wáé?c›!Š?‡æåŠç<ù?Œ'g7f?‡æåŠç<ú?ïìKHé¼?S6þþéÌ?c´·Cÿ‡?S6þþéÐ4FGL J0757.9-1514¿ÂrQ±ëõa@ë¹]"?•À:?eóSIÀ;Üèi
…•@T'ÊtX@ÎíEé]?ÌɞÄüžÍ?ÚX™Ÿ"ðp@
2Väé#E@w5Êè2?ïû™3BL¬¿áŸ
='¿é¾kÀÃT(¿îÔÚbaŸ¿ïrô^Œ'k¿ÐÚáŸÌUNASNone?ï·ü`ÂJ ?–¹¹Tzp^?'çÏmWá?–¹¹Tzp^?ØKxFÀÍ?ÑZÚ|'>®?ãÚ1Cܟš?ÑZÚ|'>®?絨gÆpï?²–¡¿à[?Д¯0s%?²–¡¿àZ?ÓjÌ(Ôç?³>v§XÏò?æJð땋?³>v§XÏó4FGL J0758.8-1450?·£ú{@sÞ¤e¥vÀ9éɼw4À<O‹À@Y{SJ?ý–ç½éÚû?ÉÁžÛÍƝ?â¶ÝÂhoÖ@Ÿ=áâއ@rÅë‡"?ßcøb|ÌÚ?ïàuöý!ÿ¿Æ:'v_'Ç¿äÕub'¬¿î"0Akˆ¿ïÿŝƒ‰UNASNone3FGL J0758.6-1451?_S¡³h?b£Œr‰'?ïðtV/&r?b£Œr‰'?"JZá•É?¡Vʤ^®.?ï®Ö"{©?¡Vʤ^®.?šú/àbª?Ž~˜;kŸ/?ï(.€üê®?Ž~˜;kŸ*?†ØñfÕ¬?rŒ+/s?卵:d«…?rŒ+/s4FGL J0800.1-5531?áúÜÕ·À*@!ÀD(NÀ:Ìá*?À<ªGfÆÞ@ï°oÉçj@ÁÅg}¾?ÉÄ
'?–%"›ìÁ?ÑXŽß#@ÓÝ¿¹>?ï"¸Ç\J"¿â@!X?\¿ê
…/J¿æBM'iҿדrãø7Š¿ïÿ'ö֌UNASNone?ïïs
zGö?d^ªü•?`Œõ…¸
?d^ªü"?ïû*€» ?aÆ/¦K™Ç?CUý½©?aÆ/¦K™É?ïw{h˜"%?‰{҆&R?''ìû»Z?‰{҆&P?ïçT])Ç?V"'`¨?h«¢ñÖ8{?V"'`ª4FGL J0800.5+3715?Ù{Áz$!@='à°«À;¶–ʞÀ=jïVd£@Q±; è@¤+eßWê?֖©ÁÍ?ïþh@0FÅ@
ˆ¹w…s@dCðš²H¿éŸù8¿å";‹ÇI¿ÈE/‡­¿çTÁ£Mø¿ìrô´rbô¿ïÿ»×²UNASNone?äšO ò»ò?ÑVrÄ?ÖË`¾ˆ?ÑVrÄ?âû´#b?ÓãMÛ~™ô?Ú	ܗ¹;ã?ÓãMÛ~™õ?äûÏ'?¹Ý­z¾ý?Ö	ùøañ°?¹Ý­z¾ý?ÓÉG҇?¶ÑLñPA»?æwܼ?¶ÑLñPA»4FGL J0800.7-1059¿ªþØى;@#ú£iüóÜÀ:Qû]ÙÏëÀ<9¬üLí@×Õë™"@ŸNìő?Æ	[ˆçÅ¢?ÅAòé—ï?ý'-K6?ü/š.êÏ¿ï²LîÆÙ?ïÇìÞe%Ÿ¿åÏ/!}¿åNžsž¿ïö§ý	«z¿ï+þ¶~ØUNASNone?ì,‡è»è?¾6†O咣?¾›Çèº ½?¾6†O咣?åÏz•ùM6?Ѥ;Î+¯
?Ôa
Ô
e"?Ѥ;Î+¯
?ëÍ;håW?¬6ŒÃ©û?ÀË\j£œ?¬6ŒÃ©û?å?)åÖE'?»+ɤ³êã?Ձ¬4Stý?»+ɤ³êã4FGL J0800.9+0733?풼ÈPa®@2ÜJ@•òEÀ;~™Pž~À<éö\é@ Ž¨‹úʌ?ö½õ<ó¦?ÖHì'õ"@?げ©@ûA3¦ö?ö~ÌôºÒy?åè阵n¿ïÏYÚféC?ïÿÊ»z"ò¿•Ã0}¢¿ãÍé,~ä¿ïïá9k[™UNASNone?îÛ_~£»J?¡ï"ƒ¸:d?¢JÄKj?¡ï"ƒ¸:d?蝰Ónr?ÒÒ¾–&â?͉<²Gú6?ÒÒ¾–&â?í å˜‰#Ù?£†ºD;©þ?²øÓ;¶á>?£†ºD;©þ?åqD؍\?Â$#
åaÆ?ÕûvNåF?Â$#
åaÆ4FGL J0801.3-0617?ê–zrmű@(èä¸{ÜðÀ:ŠS±WüÀ<s'È@ùº=S³@ ƒn—?ĝwI¸…Ã?œAí¤ø?Ö–­V?ü»%_5?ê?'—•¿±¥Ku쎿í3Ðçå¿Ë—¡ò®‰¿î#f!/a¿ïü]°	sUNASNone3FGL J0805.0-0622?îcH¸óz"?¦º¥S X?©ËtpÈWÈ?¦º¥S X?íý÷à)?Àúÿ:öuL?°Gþ·ß?Àúÿ:öuL?î8ÕÜZ§?œŠ^¹Æ¹?¬r¢:UÎ?œŠ^¹Æ¹?îAÃOÌÅ?™¥ý¶°?«îÃË3´?™¥ý¶°4FGL J0802.1-5612?ï+ñ-ŠiÀ*kQœIwÀ9ÑÈDŽŽpÀ<Wí|o½'@
¤þ&¶ù?ÿ¡Å'U°6?À]¨½#ž?èMàÞ|¢"@#sÈ:–ÔÃ?üüo'ôn¿éÉ9d¥œ?Ðû‡n…D¿Õ´`$-ó¿ê$ŸANSö¿ïÿýç!é?èAôl#UNASNone3FGL J0802.3-5610?'ŽÕó%¶·?¦À'Œ†õì?ïk‰PfÒJ?¦À'Œ†õì?ƒõÙH³ÅÙ?™"M©$¸Q?ï°(šÝ0é?™"M©$¸Q?œ¾µÃÌ!?¤Òc l•?ï
QáŸ/?¤Òc l"?B]]Ëm@W?8Í|…i˜?ïûh¨$°?8Í|…i˜'4FGL J0803.2-2522?±Í"Ç¡-C@ùݧ¤À:ãhšô­À<0ãs\@…_ KúÕ@ª¬Ùè>B?Æ2šÜ垫¿' ƒ~áB·?Ð0¥Nفç@b"¼î]k?îR¼›&b¿åîs°Ñă¿êM=Ëg¿Û!L€â¯¿Ö—†"iÓ¿à"ÈŸ@¢‡UNASNone?ïމua~?mÝ͟þng?p»EOpA?mÝ͟þni?ïõp»°Y¡?ƒ̝»?UˆŸL¾>?ƒ̝¼?ïËD9-?|‹+ÖfV¶?zs]ÿchã?|‹+ÖfV´?ïãÖ²—ëé?W´ƒ¸œà"?l)Mh÷?W´ƒ¸œà%4FGL J0805.3-7425¿×í¢=À5QŸ<pɗÀ;8rǝ¸ãÀ<‡TÂÏóÉ@x4`YÜë?ÿO²ZZ¿i?ӊÙÂÿn‹?Ôb'ÁÙ'?üµ]åŽd²@T"Uð¢¿ïû¨b4R˜?ï$‡nÊ?­âcAën¿äO
?¸¿ãÏJ ¸æ¿ïú;e0ÜAUNASNone?ïæZ¯B¼:?hN\í†l?i¥P½CÅJ?hN\í†l?ïòWCŸi ?wòI&sßï?[QxÁ,ÁÊ?wòI&sßí?îØÙ¤‰'ú?–y	~¸?¢re·fÐ^?–y	~¸?ï-ôH ?…@œš	M?šAvþì?…@œš	L4FGL J0806.8+5659¿ìÇ(.Ü@@O+ý´Ì%À;¬sè/(âÀ<ôe;Ãûm@ Ó{d¥F ?û¯W™?Ön5Ó £ä?ÅöRT"Ö?ñWE+ƒ;‰@ï¾Î²U¿ïÿêf:Ç|?ïÿx†#›¿çöˆ‡ù^%¿»ñöýÍË¥¿ïÿ‰î*ëf?ïüÓZ…‡"UNASNone?ïû‰×:ۑ?Gëˆ%Y?AØ£'»'?Gëˆ%Y?ïù²sçÌ?nÍSŠHßv?I60bÐì?nÍSŠHßv?ï8ò¬í×?v]ó~ùt?˜á½ŠbE?v]ó~ùs?ïØyè¤{?l¹6¾Æä®?sÃ8­Âs?l¹6¾Æä­4FGL J0807.2+3312?ïY;xn@=q
{é…jÀ;{ë^ˆK"À<Òâ'0ïŒ@{;B `ô@¡E= ó?Òå–È.›?Ò¢
a,ë›?þ$Ü=ƒN?ù<p>–©?ïþ âx°–?ïí5€†£¿Ë¤è'4ù¿æaµ&½Ú¿à_•'Í~¿ïû…LXžUNASNone?ïãù8Ç?t-—?wX^?låÇÿ8ò?t-—?wX_?í¢•"?¼ãŸ'GïI?²ëWÎïÇ£?¼ãŸ'GïJ?í™!#fK°?¡³é'?³6öäÍ¢?¡³éƒ?æÒ€åZ?¶¿	×p#>?Ò[Ôþ5ÿM?¶¿	×p#>4FGL J0808.3-5121¿äQÿ^S_;À#ñÆónøÀ:p1ÆK©LÀ;ܽ:ˆ'
@h`©
*
@
	Ö¶[?Çî•ßе?¹–UGì?ó~5Å´ª—@G+ÇYx¿ïZ쐰½?ïݍyЦv¿å©mƒÐ¿è×_Y¬Å¿áWÊÂ0'˜¿á2€óUNASNone?ﶓ@©HÔ?'{,š)€?'[/Õ­Êä?'{,š)€?ïÝœ6ª8?¥ÅØdÕU?‹È˜òUqå?¥ÅØdÕU?î6ÃLX?ž‡*¶M›4?¬"Ë?ª~
?ž‡*¶M›2?îDP&ˆµò?™p¸H"æ<?«ºý—t Õ?™p¸H"æ<4FGL J0809.8+0507¿ê‹µÞˆÂó@3Áõ8%á;À:ˆ$?ziSÀ<@w¯<™@iIºß™@…N{ŽØ?х¨á`,»?ëtm$ƈæ@× eeµ@	ÒG6u\ù?ïþš¥2T¿ãœ \–ÙÌ¿ìÞî7€ ¿ë7ë(Øf^¿ïúžâXÐ&¿äC<àÛødUNASNone?¨½ê"?±ß@?®8H?¤·Ut!]ç?±ß@?®8H?Ìoy-f?Òâhh#?èä!´¼?§?Òâhh#?æœÜúÇ5?³:ö#¬ì?ÒÆF
q•?³:ö#¬ì?ÎþZ¤ôÝ?¶¡b'5?è@ixÖÂÈ?¶¡b'54FGL J0810.0-0505?êu,r,@-Ùh">À;EìSzÑWÀ<˜(=5ët@h
0ëp?úÉoŠÑ€?édÝÀ$5?á¢ÛA"¯¨?ù·$#Ë·#@N²OÈë¿ïüœ¾g.b?ïåèâ­â¿ãÊh8Î}§¿ØߕÜö–¿è$½"Zm4¿ïý'!« €UNASNone?ïÍ	‰U|?|ïmËÜ2b?y{{»UB5?|ïmËÜ2b?ïi|:ˆ?ªéÉ/ñ©"?'Ð?˜¯?ªéÉ/ñ©"?îù]Ã8º?•Ú¤ùÿû? j#Ì~DQ?•Ú¤ùÿû?îBPdêyE?˜ÐPb*5?«Úù±Xkº?˜ÐPb*34FGL J0811.0-5636?çÝùs¶À(´Jb#á‡À:&Š®DÀ<öÉ™"@i¥ˆ€@«"}¨¢K?Õr4ÐÂ$Ó?Â'}mi?ôò†š¹T?þ{ZÚ6x?ïû":ŒÃÈ¿çÑ;&F»¦¿çM<>ɚ¿ÖôF£ÓYY¿ïÿJ˜ª†Q¿éyéÐé'ÿUNASNone?ïò¸…â?dg89˜<d?ZŽô;÷çç?dg89˜<c?ïcç+ñ!(?¤}8|ä·¿?"ƒÛÚü?¤}8|ä·¾?îæ(˜Ë¼o?•D¹üKo'?¡vsD9?•D¹üKo&?îÍ7G†?'•nžâ{Ã?§ã,Ž›‡–?'•nžâ{Ã4FGL J0813.1-5049¿ãù	g"À"">À:W^!ôFŽÀ;¿jК¸@}ã ÷€@ü*EMçê?ɂâˆuÚÎ?ÃùGÿóë ?ùlsßË­@·Uê™?ï_‰ÓRù¿çt¸Œ£è¿æŠP†*Q¿ì	ÜW"KT¿Õ©ºy
2¿ïý3!jˆàUNASNone?ïD`h´?™vºZÑUè?—sòÿÉ|Ù?™vºZÑUé?ïiDòć/?¦ÖÆl×?'×a§o/?¦ÖÆl×?í"?âSûM?¦CèýŽ?¶îí`%™?¦CèýŽ?î=•®#?™@T•åHR?¬&®eýÌ?™@T•åHR4FGL J0815.5+6554?æÂÙ@@'Ò^ÝÀ;Ýh1AÁkÀ=ûG3›8@!´u»îÙ?úÌ 4Ríä?Ñw~ý.?»À'׳…©?èÝAÄÆn@†újê°?ìDS­úпíđʘ?'¿È"ãw3=¿à·íu?¿ÄÓàR:µ¿Ü+Uc‰½.UNASNone?ïÿ,•:âô?!	-¼cJ[?mX£¡z×?!	-¼cJV?ïþY('Ä?E™Ì-hJ?*mÆãÆL?E™Ì-hO?ïóKÓèu?mø	//;?YhYÚ/F?mø	//9?ïûLJíùõ?5.ˆ§îÓ+?BÎÔH-ü?5.ˆ§îÓ/4FGL J0817.7-5258c¿ÑY+ë©À#:1…ýÀ:[6ÖUâ‹À;×ê¾O@8°.†{/@CºkáÐ?Úß©HcF ?ç/Xb—¤Í@Õ¸~a.ï@=Õø¬¤¿Õ#lì'dò¿Îv~6'·x¿ë–îÄnYz¿ê{åßBp=¿ïùV}»¿ãs_ÍSÛUNASNone!?ì>ðyÚò‡?Ãg¡¿ûy×?¾|1(kÈ?Ãg¡¿ûy×?ßHÉg4;?ÓLhUÄO5?à[›L}eâ?ÓLhUÄO5?äÛÂe[Éß?¼zœ –ÏD?ÖH{5HlB?¼zœ –ÏD?ÔᗉzåÊ?¶CeãRÛ?å4;B?¶CeãRÛ4FGL J0821.5-1436¿Þ.µxò'º@(×bùÊ[ÙÀ;\>GckàÀ<ï/a›M@C×Æ%ß@*,©¬6T?ÔõD䋅?íâ_ !¸@Jùe²€?û@»×‡ÿ?ïà/€ KÐ?Ú,¢'¼†¿Ý¯»/¿ïáB‡N=?êŒäIÁ2¿ïôþ¯çÝUNASNone?ç¿Ñi2˜?Ï%X|D?Ñæ€]-šÒ?Ï%X|D?ât}ñԙ	?ؼø?ÛVÍî?ؼø?׍j€Š"?¾eÁ›ÎÂñ?ä9vÊ¿º¶?¾eÁ›ÎÂñ?àþšØYf#?Ð{V(˜±?ÞÊOM3¸?Ð{V(˜±4FGL J0822.8-4207¿ámR_	 žÀ±ÕQ֌À:4®'xbèÀ;twlH(@!fø1ªr@ÆcÉÓô?Ç^«œ{vC¿ VQ›S-$?֜TŸi'@@X·ˆB[¿îø–^ü³?îqBÝöð¿Ýû
'ç¿¿çô¯¼пЈÊÿÃE¿Ø«úú݁PUNASNone3FGL J0823.3-4205c?ïö—"=Z?Vö>ºÆ-D?RÐ×ӅL?Vö>ºÆ-H?ïùAˆä]d?}ã½¥WJ?JùÜnŠn"?}ã½¥WJ?î"Éûy1? ¤ö|{aà?¦Ã`Hlæ3? ¤ö|{aá?ïñ|è@Ëç?TÑWE$~ª?]/~h1Ñ?TÑWE$~¯4FGL J0824.1-6004?~2áì~rÀ)wùÖñýÀ;W†Ç.þÀ<ªZÉz1õ@!ÄÀ:Çý@üÑ\~†?Ü
ËD·j?ïÿ±eh@.Ý}ôøe@Jöô=ª¿á¼œ2Ñ
¤?åRqâpx
?·sëÇkd?îÙ²X­@@¿èù"»¼Q¿æ‡Œ+ÕqUNASNone?ì@\¦è¶7?¹¨Þѹ&³?½ýȺNJ?¹¨Þѹ&³?ìeRšÂ:¦?ˑҀ‡Ò?¼Õk)î*Ò?ˑҀ‡Ò?ìיÐr¯?§	–lø;?¹C1|oò'?§	–lø;?見'Ë°?ÁVʒ¥l¼?ÍeÑôÑ=Ï?ÁVʒ¥l¼4FGL J0825.6-5216c¿Èä9!&pÀ oŽ\NµpÀ9¿MÈ	ïmÀ;Š
öÔT@/A:2@'âƒw?Êy@ˆ±>ý?Ó¶h\_ÒN@Ç>Ê€Â?ö#õ¶6ˆ?à*ڟg¿ß]e¡DˆÆ¿ê¾'¢O¥¿ï'Iž¯ƒ?«ØSœ<ê ¿ï•Û¿-ý¿UNASNone$?î*I­ÕP?·Ñ ØÓX?­[nE"ªô?·Ñ ØÓX?è‡Gâ»î?ж¯à -}?ÍâàuÐJ?ж¯à -}?㋵ÍlD—?·¥Ï‡LY˜?Øè"e'vÓ?·¥Ï‡LY˜?ä'ì«åŠè?ÅEòsSÁ?ÖÜ&¨4ê/?ÅEòsSÁ4FGL J0826.0-0157?ï§'§G*@3öˆœTÀ:­`#VF^À<u°ç"øp@ÜÞ'h#Ö@DÙMä?Åßïÿ¬Èö?³íDfŒQ?í./ˆƒÇ @ª6+‡m?ïýI1¢9¿ç>¨Fۆ¤¿áüHKá¿æøÒpXƒ¿ãÆôµ¿ïÿÓ?,» UNASNone3FGL J0825.4-0213?ïþ>ÌL¸?0DU(ÍW?,s;4~"?0DU(Ín?ïûŠ#iÉ?_	ÅÍ·¢
?A‰×rXÞu?_	ÅÍ·¢?ïؑr¢¬?th.'˜ïË?s·Fó.©å?th.'˜ïË?ïމ	àf?Y˜ŸÔEs?p»1{Í?Y˜ŸÔEn4FGL J0826.1-5053¿îÔ68ýÞÀŠòQÁ"´À9ÝË£!hÀ;©Ââæ@ž3×Ú@I6'sg?Ä!Z˜§×?АA–£E@
Ä.bT@kK
¶!¿äïv_Ø­¬¿æðÉ+WœŸ¿Þïeþâs¨¿âŒèæÞÆÊ¿ïÿž ßt¿è««Ÿ«yUNASNone3FGL J0826.3-5056?Ý9"A|?Íd'"7?á~c6_uÂ?Íd'"7?éo¶øÖG"?Îp=ÏÞ3­?ÊA$¦áð?Îp=ÏÞ3­?Õ´@Ümg?¹E	J@M·?åw¥ß'ÉL?¹E	J@M·?è·7'Úî?°"C˜6Ç?Í#«!¸"L?°"C˜6Ç4FGL J0827.0-4111c¿Ð0îáEã¿úköÉ™"À:"'‡V ÷À;‰Õ¤â¢ø@!«t0Ô^<@dïmâ?Î`R»Ž¶è¿ŠÄ©Šô¯?°:³ží/]@+áìõ?ã@JÞJ£'¿ÛçÚDY¡1¿é°Úþ¾·¿áírÊ!÷¢¿ÂN9žÝ%`¿ß¨bÑÜVUNASNone ?ïلGœz4?t2qò¹JH?s=Ü1Âåá?t2qò¹JG?ï÷@Hµ/?'ã¡œS?Qo╢§?'ã¡œS?îÀqÀø2'?™ª&â"A?£øãð|ÖÓ?™ª&â"B?ïà,}
š˜?dY'9,›?oӂõehs?dY'9,˜4FGL J0827.6-0059?å~—dõtø@4Å2¤—ú]À;lWÛÀ<™ã½ª@ 
ããê¡?üe2.?ÓÓMÅZ½'?Éۥá|?õªŽI@Öې	"?ïýÐ_ÿD¿ß:Ç|*óÊ¿æAIvk—(?¯Kì_ÁW¿çIéXÎG¿èsHÎ÷ŸUNASNone?ïÿ ¾¤5ù? cÄ×?è+y@äÌ? cÄÉ?ïüCzqa¥?X=~vÁ2Â?=ä,tòØ'?X=~vÁ2Ã?ï·ÜOxE?€àÞ_¼£?'ì!î¼I?€àÞ_¼£?ïí욗3Ü?P `Þ?behÌ$?P `à4FGL J0828.4-4444?Âù^7
͵À ¸Ý+¿¡À:|ÀØ£À;Ï™¹z
@ ÔÊCX@é@&?Ïø‰ÿr¼`?ë:I½cMW@:ð
­@]"N+1¿è¦î·`-¿íù䒼/Ç? ¼«³¿Ý±cºº|¿í½tŸå
5¿ïÿþÞ÷UNASNone?²VÔlõAú?ÀÅѧÐ?íµ%raWÁ?ÀÅѧÐ?ŗ®?¼¨?ÍBV'¢†?êšpÕÜ?ÍBV'¢†?ÂÁMøI?®ÆAþ02?ë}þO¬î?®ÆAþ02?¬aL‰½f|?›¾Ê¯«õï?î9ë7d)™?›¾Ê¯«õï4FGL J0829.3+3729¿ã¥ö!—'H@A`mqóbcÀ:Œ»NŸ À<xÉÓI@§6õŠ†+@0ïVd£?Çá£Þìßè?ѐíBäE@Mjßqêÿ@ì؜¹´—?ëG™ò"í¿å¥Ì­ÃJ¿é¥ß™±¿îå7&ݺ[¿ïµ6þ™Îs¿àЏ¥UNASNone?îp¶îÛW?ªÀðeMr˜?¨ô'JÅ?ªÀðeMr˜?çJlÜt¤?ΣÝx¼Bì?Ñk&G¸?ΣÝx¼Bì?éüSZú€?¯Þü
I¤ã?ȳÎ"?¯Þü
I¤ã?åL˜Ðy?·d8©z­?Õ×ÝfÎ_?·d8©z­4FGL J0832.2-4322c¿àáµÛÀ<œƒXåtÀ9˜4¦Ð¹ÁÀ:‡l¸K@ ½[8á@½·B÷ÌU?ÊV/wˆ¿g$b­@¸?¹í•W?@YBkàMÞ?ïü÷™Ã
¿èË÷º·!¿ê…ñxô¿å MÈ௿àùã»üšñ¿è!,À¨QBUNASNone3FGL J0832.8-4321$?í·Ía]X9?¼!ƒ7W?²A"õ>/?¼!ƒ7W?ïӃêüL?Ÿ­™ÚLš½?v>
öÙÃ?Ÿ­™ÚLš½?êW!-´?´'Ÿp³?Çú£{I/º?´'Ÿp³?ïnVÀJ¾ª?ƒŸÙÀæXn?'5'ö¨*Ä?ƒŸÙÀæXn4FGL J0833.3-4342c¿Ä¯àß×À—)|Ñ÷À92\ça£‰À:T@ ¤		>@Móùa€N?âÝÄ6%Uû?Ôñ†U7	?ò&˜Ö%;#@í‹k®yÐ?íYÌúïõÇ¿éPCD"nÀ¿é$ó¿ÕÃk¿ß.^b6¿ëÏ*à~Zy¿æ‹¿m"¬UNASNone ?ë‰Ð×V?ÄUà™ª9?Áۀ¿œ¢ª?ÄUà™ª9?ïïKÁä7h?…Ü`FÄ?`´>ȗL?…Ü`FÄ?å÷é—MÂ\?²Ž‹^uºO?Ô,Ñd{H?²Ž‹^uºO?ïYh'ä6ö?‡X`{éeE?"Òï£y!C?‡X`{éeD4FGL J0834.9-4612?ìÞYHO3À¯"9櫛À9G6v¾À:¯"½i'@ &K¿ÆÿÙ@q̾Šë?Ëjß\qp?¬)œÜo,3?å¡ä¶Î^?þö-pülx?í4T€ŠÔۿ뮛‰]â3¿êj •6^¿á?&¼,k™¿ëPݾ¿¿â†œ1#Ž{UNASNone?á7±¢ÁÖx?ÐㆅÙË?ݐœº|S?ÐㆅÙÊ?íÔˋ ¶¨?§ñOq ¦?±Y£¢úJÃ?§ñOq §?åO¨±K¨?µWäË&e?Õ`®õh¯?µWäË&e?æ¥.(ÿó_?ºzÜò\¦?Òµ£®B?ºzÜò\¦4FGL J0836.0-5458?ÊÌÂØfôJÀ!	(¿;ê'À:SEùßTÀ;æÂW(@A&œÍ@ˆ!¢7?˘iñŽM?Áøü–'O?ô½áâއ	@Ûr±Î?ä•qì¬f%¿äègÝßÄ¡¿ë¢_:øú¿ã
+Í
dm¿èÕøÅy¿æ¤O QC¿UNASNone?îÁÉÏÆÍy?¦k.~²u?£ãc"(s?¦k.~²u?ï0)qÀj?¡!¡öíÃA?³õ£åŽ?¡!¡öíÃA?í‡R¯&–?¤÷Yyµn?³Åj‡>ËS?¤÷Yyµn?Pýªw?Š¥ˆã´H?¤fzð%X–?Š¥ˆã´H4FGL J0836.6-6036?ïÒÓ,‹À'õûmÊÀ;ĘÚÀ=Q΁ز´@ÙÁ®‹™&@'$·omv?Ùè—ä7Íw?ïÿºà¼ô@zœ™(Z'?ó¶Yh|O?ï¬;ݦ¹¾¿ÑÏ£@âH_¿Æº–ê<Ê6¿Ù£C;"¿ëØMú^Ö¿ïøg_µ0UNASNone?êhì¤ù,=?ÆÉtPÓS¦?Æ\MlO?ÆÉtPÓS¦?ÓÈ«"¨}?բƵÉK?æv›ª6+Â?բƵÉK?ä¢ð¶×ôÓ?¹h#ã"ZV?Öº'PY?¹h#ã"ZW?"?À\F•?'n~Ԋo?ïfýËS?'n~Ԋo4FGL J0836.8-4638?ᓋSƒTÀ»Ä?_'À9m.Y°À:°ËJì\@êv¹DÚ¥@<G䛬?É@tú¨Ó?²µÔ¶a{?硅‹Å›€@ÑQž?ïò÷ÙÀÑ¿í
°'z˜M¿åÆ ©T¿å³Æ)ñk¿æÁqN÷´Ø¿ïÿÊ»z"òUNASNone?ï¾*9µ?‰ëGÒÆÔÞ?€uq'» !?‰ëGÒÆÔÝ?ïãqÄNÇÒ?—Fòagî?lŽ;±8.9?—Fòagî?ì]»€ÊÊ ?®u§k¶A?½#ù©¯?®u§k¶A?ï0œó§{¨?ˆ¥~Ë©?™ìa‹‹?ˆ¥~˪4FGL J0837.8-4048c¿ím@#T?=?ˀ.¤SAÀ9M1áú[À:µƒßóðþ@~;Å(@6¦Bˆ?Ç×Ñ7À‹¡?Æ$£ç"@߂±ö‡±?ë`s/¢"û?ïýAԋ³¿äè]_V¨¿çæ끘Æá¿ësP$¿ð?ïÄT=nöXUNASNone3FGL J0838.9-4056c(?îGîÒT?½Áþrì7c?«Ž!Ú¿ƒ?½Áþrì7c?äK_ŽÇNN?×Ã9D?×i@âqcf?×Ã9D?ä;|nË»?¶UQî
?׉"h‰?¶UQî?·•å&T?¨7íC6è?í
^#[-ö?¨7íC6ç4FGL J0838.4-3952¿Ýø¡ªÄ§K?ë»'ˆÛuÀ9yo/bÄÀ:Ó¥á¦x¥@˜é6ºÒ#@ÿ^Ö?ۺϟ:~?ãqbx›Q@jl»=¥@"©ë¡ND¿àq¶ùê¿Ü&n¿%oP¿ë²ÑCT§¿ìÕwácà¿ïûJ>³‡?ïë/=Û,âUNASNone?Ýû¯z7‹K?Ò$qW‡u?á(Bä:Z?Ò$qW‡u?Ý0§€Â˜u?Ö½(عƒ3?ág¬?ž³Å?Ö½(عƒ3?۟õøåâ‡?¶6¯}P]n?â0»?¶6¯}P]n?ÆÔ,*\8~?¶šîYîþ?êJôõhñà?¶šîYîý4FGL J0838.5+4013?æ|÷ȯ˜g@Bt# –x}À;žU9xÃÀ<Ò³‰.èK@"Ztâ*,#?ûA*ØÞ©?ÆʙÁ²'d¿—…ã{²Jb?Òr>¡ÑL?òh_ōh^¿ïÿÿ" 5•?ïÿnªØ†>¿«2Zp8ø¿åÍ}å¿ØÊE¾¦ƒ?ѳžþ]h'UNASNone?ïýӇRõ±?5Õ÷7â>?1cÅhRx?5Õ÷7â9?ïچѧ(œ?¾îMQÝ?r¼—,k²\?¾îMQÜ?ï±h04ú?'yFþx˜?ƒ¥óüòÁZ?'yFþx"?îêì®Ô	"?'`Pv«;?¡Q5¿g¼?'`Pv«;4FGL J0838.8-4552c?ê­TƒÿmÀ©Ðé'ÿqÀ9]U÷ƒY¼À:2`Nq@ o]µ<ã5@—¿|'1ž?ß'kŸ
qÉ?ìÃ-±@`Æu(@qÕÛ>U¿Ôºªö¹/a?ê_ä¡Õ¨>¿êvåں̿ãá"ßþع¿èEÓI¿ïÿÙÔóüUNASNone0?Âÿ²©u³Í?Ï
x-'‡?ë@U¢"?Ï
x-'‡?ášþ#"L?ÕàW±Ô.?Üʸ×g?ÕàW±Ô.?àC—ÿT?·\ù?{z?ßxÐWÏé?·\ù?{z?Ë…S>˜?½ÌÊ:%?é8«0z?½ÌÊ:$4FGL J0838.9-2502¿íÀfԏðô@#¿¸jßÀ:ˆ[3,}7À<GĐ¾(Å@æ)ÊÔ¥@ºñ¾Ýa?ÒϏìTR?Ùz®ƒ?ýçdã¯ga?õL®Cõ£0?ïøbaô瞿àpLÎå«Á¿éí{˜ý'g¿è%LÀ¢ó¿ì'¬Óª7?ÖÅ|vs#äUNASNone?ìÕ2¸L‡?¿ÿ˜F‡1?¿Vj=›É?¿ÿ˜F‡1?àtšõÓ£p?Õ/¯'ðÒ?ßÊX¹"?Õ/¯'ðÒ?ç®Å¯Pò?²º1ãJÙé?Тt¡^à?²º1ãJÙé?͇¸çùa!?µhOTc9q?èžÆ§·?µhOTc9q4FGL J0839.1-4613c?ãÚ¾§º'À>‰¨‹À9q ٔ[lÀ:ªi³øÀq@ ¤ù9@FE^¯?Í'ØŠE>?ËHoÛZ.J?öñ§ãxu?ùSj…ÚÊç¿îcϝ·‹r¿ì "@º?î፞¹"¿æäW}•W¿æãyÌz¿êøsCÄ{UNASNone3FGL J0838.1-4615$?ä_'üÄ-?ËS𪖦:?×AÚÜw¨?ËS𪖦:?íS_^n=?ÇȪ'¬53?·
eŽ?ÇȪ'¬53?ãfg±
(?¸*îú!?Ù3á0ë°?¸*îú#?ã|½†z‰¤?Á˜z¾:—Ç?Ù"ó
ì¸?Á˜z¾:—Ç4FGL J0840.3-4544?éÒ¹Ë#íøÀp²˜À:±èkŽÄTÀ;ºB<»r1@#'½@è¨u?ý(&¶Â?É£{æÖ¿—çÁ<BGð?Ñ3¢÷¼:@ŠF~¾w¿Û¢<€cé¿ïùÔØ4	?ïgÖs>»ý¿àÔ&~ïʿ嘑AƒÍ¿¥µna\'PUNASNone?ïúbúWñc?Dm'[⁄?Ft :vZ?Dm'[âz?ïçd_2ñ?›shj"2?h›ê Í?›shj"2?ïCÜ"+§u?"<V<JøÓ?—"{º‹…?"<V<JøÔ?ïºyA¦æ??€
ãÌ÷Â)?a¯–Fp?€
ãÌ÷Â)4FGL J0840.6-3130¿×›Øtkf@3Ð9h×ZÀ;Ué'9YÀ<ׁ›v¬@'1È$@ü.Êî¦?ÖÜAÿÿª?íøЁZ@ñ¯:ÎÄ@
$ùS¿ïþÊá:B?ïXÛch…?ݼ"C¿‹¿èÐMUhÇ¿ïÿôÕ÷?îb¿è¸¼UNASNone?Ó`-/+â?Éeé}|]?æOéhjp?Éeé}|]?Í —Žœ?Ñ$Ä2Ù?è¼WÚ:ÜY?Ñ$Ä2Ù?ØA^›Óžq?½ƒÕ$°K?ãßP²0È?½ƒÕ$°K?Ë«¶ʁ·?µuL}¹?é{Í_'?µuL}¹4FGL J0844.1-4330?èr-d½8:¿àíQÂjs;À9Zox]߯À:š‡–ü@Ãay@ y½[?Â?ÎàÀʊþ?ڂZbÌþÌ@
RÈ>Ȓ«?ûæ"KÑ吿ºÐûۃ¿ëéz'}¿ãÌôÀ0Ý¿í:­³N¡¿ïÿ~Ù#ó¿ïûR¼ev|UNASNone1FGL J0845.5-4327c?Öñ7ë®?ÍRÀ~÷à?ä÷‡d
xª?ÍRÀ~÷à?ÖP
¡j}?ÕLú—v¨?ä×þy/JÁ?ÕLú—v¨?Ð$¡	L´ó?³hõꇒ+?çí¯{Y¥‡?³hõꇒ+?«¦"$h^E?"\ÍDsˆJ?îEÝ¹z?"\ÍDsˆJ4FGL J0844.2-4554c?×tö¾·Ú¿ÿùyÔttÀ9N:¶~­À:³>Áï-@"#êÀӚ@
KáQ?ÏFªâ?уZ{w?ý«·ùÖñ?þQvg]?îyÞon¿å<5œ}z¿æe墆¨%¿çœ&;Ó륿åéÀ°3å¿ïÿî,˜å?UNASNone3FGL J0843.1-4546,?煏4 ¡¡?Å:è™@?Ðôᗾ¼¾?Å:è™@?êNpËN?̙ññ/Õ?ÆÆ<ÓúÈ?̙ññ/Ö?àïãIB±?¸²Àý70?Þ 9mzö?¸²Àý71?ݬÐ:R|Ã?¶6Ìå)‰v?á)—âÖÁŸ?¶6Ìå)‰v4FGL J0844.9-4117¿æP¦•@;?ï l¡éÊ4À8ôÃóà7
À:ËeCP·¨@¤d[Ÿ8@±a£Êu?ÁSŒÄôç?Ò`…_@V=>Nð(@Qï x¯?ïÚ¨W¢~E¿Ú"uá-¬á¿éÃ}Ò霿èØRq¼Û¾¿ïÿÿ>¹ú?í쉖WZUNASNone?ÉQÐoš¡o?Åüp©Ø?髋äW¤?Åüp©Ù?Ò´j²Ÿ?Ԣ̿ƞL?æ¥Êø¦°u?Ԣ̿ƞL?ÐkV€ÉF?³ …4
/¼?çÊTó?›]?³ …4
/¼?º´è:4"Ÿ?§ìîÍò5?ì©bø¹m‹?§ìîÍò54FGL J0846.6-4747¿ï?[…ºïÀ½g\/«¿À:€vÙ{0ùÀ;¢&äpX@!	¬&9%@|Ą(ï
?Â"O5G_¿µÅ3{W3?ó²"ý[
@T€œGžÐ¿èei|Æ¿éƪß<;¿êúŽÜ§5d¿Ù}®A~6¿äCt~­0¿Ü.Ë$V žUNASNone?ïí†w˜?:?bEßå±Z?byˆgÀÅ ?bEßå±Z?ïÖN3ÞIi?š÷ð.BO?tØæÛK;?š÷ð.BO?îë¶rÆ/ç?—Gœ6Ä-1?¡D˜Ó†?—Gœ6Ä-0?ï'=h 0?€pƍŸ@?‹p¥×ùô?€pƍŸ?4FGL J0847.1-5954?ïý‹xgH<À$••ÝLvÑÀ;cÉ
ûkFÀ< ë'+@!Ù0*Pš?ý«¤C@Çp?Ï-=û¹o?­Çƒêó:?âéóN@Ö?ÿ6±Ú~?»Ò6T/=¿íê͈ê?®%CÜMÉ7¿à¼{Eñ|¿æ¨ÊYUì?ÑÞÖO,þUNASNone?ïÿ+b£Â?'Ӗ?G|?"«ç¸ª?'Ӗ?GO?ïøÕL@¿¶?iê{+´?LªÎý'u?iê{+·?ïïÈ×cš?hH`Ð?`7(œeú?hH`Ê?ïÁˆ"0ÄÙ?qYXü=P?;î睓8?qYXü=O4FGL J0848.2-4527?Òs&"'F¿ò´óý">6À9OðøûÿÀÀ:ÚßVø4@a±U¢ô·@C›0r?ÁM P+?» 'ÛŠ?Ò2ÚÞ2zÒ@ìIڔ‹"¿îƒ¿<ÁQo?ïéªS%A¿ç¿6ÁÞ[¿ãâ¾°ÕJ¿ê28A:
¿À\Þ'h#ÖUNASNone3FGL J0848.2-4524?èF¢éù"?Å¿w6 Î?Îåt[¸¸?Å¿w6 Î?퟊‡Þf?ƝßTP
N?³«Áˍ?ƝßTP
N?èÌq;T?³úëzR®à?ÌÎ;«â®?³úëzR®à?íq+ÆÎv?¥Ó
ÿ\Ê?´v§YɌN?¥Ó
ÿ\Ê4FGL J0848.8-4328?ï]ü½ÄC?Äñ€uÜ%/À8UëºÎ‡À:aŸ®†¨@ƒv‹w—ç@OÅÛAÖ?Áh™ Öd?Ã[#§¤õ@K#@¬	YBg?ïÃ>Ò£¦?â®
ŸOæó¿ê0dKÙó&¿ê†Âùå¿æ¦òèÀHZ¿âÌø6#
UNASNone2FGL J0848.7-4324?½`ÊMƒÔr?Ę-Ђ¥6?ìSæ¶O…r?Ę-Ђ¥5?Âàlæ3D|?ËèŸRE?ëGäÆs.á?ËèŸRE?Õ
j,1ß?¿9ìO4º?åzñJéç?¿9ìO4º?¾Ðõ,\?¬!¹çç#?ì=EáZt~?¬!¹çç#4FGL J0849.0-2702?ëýt
…n@$óÛYXÀ:¡µÿ*íêÀ<*hþÇÜ@)=Úù@v»cýM?ÍZ÷¾=?Éë9ÊQ}?ú¡:wË@ÙùŒÉQ˜?ïûÜpêN¿ç©µ2&¿é/ýS}U–¿å7ÖeÒ°¿ïÿt¿Å}M?ÙÈÞÁ
XUNASNone?流©=A?'¦±Þ(ÿ?†U°¯¸ô?'¦±Þ(þ?íîæ7¿=ú?Àûê†3¶š?°ˆÎB,?Àûê†3¶›?í¤HêS%¶?¤VÚ"³±?²Ý¸­fÒN?¤VÚ"³±?ï11F]p?ˆÝ¥íu›ñ?9Ù×4R?ˆÝ¥íu›ñ4FGL J0849.2-4410c?íx'à\¿Ìl‡g½ÔaÀ9ŽËŠ­mŒÀ:ž¾®üØ-@Èíº@òâÆ3U˜?Ú®4Ã?©újꯋÉ?âÁ@Âgîý?ò²jž.~Ã?æ¤ðzPþö?ã²ç®6¿æ]Ç[sÄ¿ìÏÿ‡4<H¿¢Æ¾bHA¿ê\›A9†4UNASNone8?äi-LèØ?Ѓá-9Õ/?Öá-¥f.P?Ѓá-9Õ/?æö5.tÔC?Õ̕Ô­Ê?Ò•£W{?Õ̕Ô­Ê?åýOyl÷?¸Gà£ß?Ôa
&ß?¸Gà£ß?ä@–jÒ&¾?ʚ±·uN?×~Ó*[²'?ʚ±·uN4FGL J0849.5+2710¿ïé=˜3D@B`'ݽµÙÀ;:I¥ÒÀ<š…&E'@Ɖˆ*@ þG™Å?Ñd}£Cç`?ÊÙ'#0?öS¡Qô¿@ˆ3û°'¿ïö
~C›?ï•Z0Fð¿èªq"'¿çq'úä¿ëK»%_5¿ïÒŽXUNASNone?ïã+Þ¯už?q¸ÉùNœ?lÔ!PŠaû?q¸ÉùNœ?ï÷ˆ'/'~?qX
"qÌv?Pîû ûƒ?qX
"qÌv?îSÒÃœ¾?š,{™Q?ªÂÓÎæ4?š,{™P?«^î?yDpŽøö¸?ˆ:U(DÓ?yDpŽøö¹4FGL J0850.8-4239?êï:)»? ¯ø×À8È.¤X9}À:OfµN+@ÿ¬)Ü@	}î$nt?Í(+Zå?è}´'l¤@«y"O¶?ù²¬Ñ~¿Øs©ÏqÿÙ'{#â³>¿í*¶W?ö¿ï¬¦Q8ø¿Ý©y¡Á¿ïçÑ­ÝUNASNone3FGL J0851.4-4244?ç×àùˆ6±?Òü©oµ?ÐP>?Òü©oµ?¶c­Å!?Ç—ŒÑ¶?í3ªG[Ï?Ç—ŒÑ¶?Þgׄï·?º:0ÁŸ(Z?àôL=ˆ$?º:0ÁŸ([?YgéäõmZ?]Y=Ë(i?ïóL
…J?]Y=Ë(i4FGL J0853.1-4407?æ2<	rüp?ֆsa¡…¡À9pNŽÙL7À:ž¢¶xÍq@åÿjþ@Œf«/Ä?Ð%lZþ?áf¦ÈVE‡@ÑÓ¾X•Ã?ÿbÄî‡Å¿èØ?ò‰J¿³ÓÿÆõw¿æ%"CïC¿ì(¬A<
r¿ïÿ|¢gô[?îÜ'éSQUNASNone3FGL J0854.4-4404?»5lãQ,?¾Kñi¾Gó?ì™]Rc•Ú?¾Kñi¾Gó?Ð 'D˜;Ý?ÓÔz6F™?çï¾Ý³â?ÓÔz6F™?ÀÒè¼4x?«[nÒjv'?ëûËEÐòá?«[nÒjv?§¶³Üþ?š	'Ï%?îŽ4"Â?Á?š	'Ï%4FGL J0853.6-4306?ïä¦iƒE?ñ%ð¥)À9
OH<¯´À:'²jJ÷@RÎؕ­Ò@ʁ~áS?Éj )?åÂ:¢"=@I!ßyx?ôIYˆ²l?›ƒi+'«¿ÖO'Ÿ,*«¿èeàš	+"¿îÞ§ msK¿æ©n)©G¿ïù>/GìUNASNone?ӎqÜ[>?ÑÂqf®?æ8ÇÒ`ó?ÑÂqf®?¥ÈÕo~?¼ù¶ÐSi?î£r®Ù ?¼ù¶ÐSi?Òùª+ÊXÇ?»ˆIÈÍ?æƒ*êӝ?»ˆIÈÍ?D°É6¸?<–CC¶èÚ?ïúؓøM²?<–CC¶èÚ4FGL J0853.9-5501¿ï¨Å¨öÀ!º^5?}À:¡îM¯À<
'Á8D@ºSç2Ԕ@þtYœT?Щ•$¿Òé?Ñ*¢ëÒÌ?üíV•8	@ƒt¿±?îûa3v¥¿áÖ!_K?¿äK›^ëÈ¿ç&#€7ÈĿ런9F¿ïöI"]ÍæUNASNone?î;ú¤b?ªu—…Qç›?¬@U¹×ïH?ªu—…Qçœ?îÚM¸Gª?·n%kƒ×?§â[${…Q?·n%kƒØ?èO~¡úK?³ñUÝMX	?ÎÂ{Ó?³ñUÝMX	?ë\,dr9?¤qµ?Nn7‹?¤qµ4FGL J0854.8-4504¿Â.ù±Lᐿ¡MŸßȖÌÀ8"Š'¾ÙÅÀ;H"ÅõB7@üíåKHÔ@
™#R ?´7¬"ž=?Ý/0ÓÊ@#ƒn—?üL+ín­Þ?êñ"¢A]î¿Û£iüóÜ¿Ê÷Ÿnc‹¿ã´k!a#±¿í]¶>•çÞ¿ïÿ³^¼£àUNASNone3FGL J0854.8-4503?IìßZ?;§0Qޘ×?ïù¸ÄÈ<é?;§0Qޘ×?iÓäe¢`?'r2¨«H?ïæñ,š^?'r2¨«H?"¤­íüß¾?nL–¥ý¼?ï­mHH?nL–¥ýÑ?sÅ»€í²?i‰çyÈò?ïÿTaÒ#ù?i‰çyÈò4FGL J0855.0+0720?â»tŸ²½›@>Åé\îÀ:Ã<«ùjÀ<\R±}»î@
´t:å@¹™Üµx?Èx/çyKp?‹Ì*IP?¾)lµàÍ
@ԆλºV¿Ìєݝ)œ¿è|u éY ¿ç[i³"¿çêï͂Õ2¿íÁ¶ÿ0![¿ïÿï9_JUNASNone?ïñ=»omC?\ÒÃ3¾}?]"‰!%{/?\ÒÃ3¾€?ïÚ27w?¾e";¡?ræä{üDÁ?¾e";¡?ïžrÓ[ë6?'Ì'¶u'?ˆcK)2g?'Ì'¶u€?ï¿q2Ù©ø?ld«OºŒÝ?€#³I•ê?ld«OºŒÝ4FGL J0855.0-6026?àa*•|²FÀ#µKjaªÀ:Ï,?#+~À<U™OǾp@Xš]¹Ä‡@ôº¼ÿÐ/?ÏGRúν¾?Ñ*ò‡qxé?ÿV­ÜF½T?ÿt'Ln¿èã'Á¹m?í£†ŒG!¿Ü~óûå¿¿âò(؇¿éÔÈ¿L½¿ïùé€aº/UNASNone?~Ü/?¤Ä¯e?§×ø=?¤Ä¯e?î'NXu\?´3#![ø?¦ÛŠxªI?´3#![ø
?듛À·')?¨
ðöF?Á±ý!÷[?¨
ðöF?êÞs4Ý®?ªZË'b½?Ć3,‹…G?ªZË'b¼4FGL J0857.0-4353c?ޚxÈ).?ð'Ú:s™UÀ95–4ŠKHÀ:}NÏpëû@¿ÃJB~@6&}BJþ?Ò#1=9ÇL?Õ¶¥ä*·d@۔XÖ[?üo|½?æö?ìåÁX¨8¿×"›¾7Ô¿æ"Mºö ¿íG¨€gC†¿æ4óý">6¿ïÿ
Çhß½UNASNone1FGL J0857.7-4345<?Ù?ÅÛsY?ÑøËdËD?ã`FT?ÑøËdËD?ÆfHq¢ÍC?ÌÅDdü³!?êfmã—L°?ÌÅDdü³!?ÑMÞråó™?¹R"¢ÜØ[?çYƍ3?¹R"¢ÜØ[?¦È¬Òñî§?—BN¨yf?î"u2Ðá?—BN¨yg4FGL J0857.7-4507¿ßpàô)=?Ôð°lCõùÀ9_É'%Þ·À:¯"¡@ÿi«kG@%³Æk‰¼?ÍÙB¼h%®?­N—½¡a?ýäJ|ûÔ!?þ`Z³«¿äý ¿¨¡õ?ï
}—"ã¿ëfx¿âyì?®ÁŸ¿î–#ùŒ|¿ïÃOÀ²0UNASNone?Ó	"V??ϚæM«??æ{~6Tòà?ϚæM«??ÅBá,JÜÁ?Ì5k,8€£?ê¯G´íHÐ?Ì5k,8€¢?â'éÈm?ºªYäٍÍ?Û°-÷ôo'?ºªYäٍÍ?Ó¶Té©gR?½"žéUZ?æ$Ջ+LW?½"žéUZ4FGL J0859.2-4729¿ã×:@?֋¿ðn*¦€2À8ŒÓa;";À:'
—~6@&®¥Ô@Âä›ök,?¶À:Çý?ÅÍÛÕÿ%@
èþüÊÁZ@ße»Æ•?ìäÀ™+¶¿ÚŠžc˜V¿æŠâ¡ö4z¿çì2"'û@¿é"¤!²Ø/¿ëbZ¾ž
UNASNone3FGL J0859.3-4732?­<œvç͖?°x‹ã,v@?î,68'ƒ&?°x‹ã,v@?É©‰7þˆò?ÎJ1'v.«?镝²]Ä?ÎJ1'v.«?и	õ$Üí?¶O×jœ8?ç£ûm'Š?¶O×jœ8?¹"X
VxT?ìA©#JL?ìÏtþµ0ö?ìA©#JL4FGL J0859.3-4342?×-r$èó?÷]qËväÀ8¤ç2© xÀ:Š·y¥@‡BÈÒlI@쭀k`?»@|`½sØ?عïºãkJ@9#'Õ?ö‡ÌbCÁ÷?å°8!Y–õ¿ß|÷7¢L¿ç\ž ¼ã÷¿êWÕÿïýÄòã¸?Уi&4G/UNASNone?€ï<'PgÞ?ô'M…?ï¼Cb¾`?ô'M…?™è¿Ê©?³4ÕÙ!Ì4?ï0º«·?³4ÕÙ!Ì4?²<'2}?§ì•‰Ùå?í¼Ø}¹°?§ì•‰Ùæ?=Á…ü€'^?-Þ{UA?ïüGÏ@oû?-Þ{UA4FGL J0859.8+0053¿Ï—¥º0ÿ;@<®Ü]cˆfÀ;9!‰½"À<¸d(ž"»@"¢ªÜâïy?Ô*"}ÙI³?íEÝYâÊ?ïÿÕ7ÕYc@žÁÁÖυ@B)"â?ì»m߁…Q¿Ó–Ñþèk¿ïÿ4Þ®÷z?ïñ
žÏ
š?Ù·`9{¢¿ãÊ?wåUNASNone?ïÖzú;R?¤ÿyTuÿ;?œå0 ¸•Ä?¤ÿyTuÿ;?ïûm±>°³?dÞO{¶Å.?BI;=3¾?dÞO{¶Å/?璘'S?"ûO??+
µ£?"ûO
?ïúSJyÜ?Q°Ø[UÎÒ?G¦²ÖŽF?Q°Ø[UÎÒ4FGL J0859.8-4530c¿ë®Çâyù?Öù¾'BÀ9.Ž'uÏÀ:§†S€@O›æ¥ç@¸1ôo?ÔùAÀÖÌ?î¨Ä_@x@£ßm¹@ÿ?þN>&I¿Ê"ù#—ß°¿ÅuB⨬1¿ígß7]¿çڙz"¿×¼Zcα~¿ïûï¯OäUNASNone1?¶oÓÓÙGž?ÀÄÛkxö?í2…"×?ÀÄÛkx÷?Òg¥_ÓG?Ó½¦Ÿê­ÿ?æÌ-P\r?Ó½¦Ÿê­þ?؂¥Ráw™?¸VÁ£—®?ã¾­VD3?¸VÁ£—®?°Ua¶ö?«ÄF]DþÓ?íõSÞé?!?«ÄF]DþÓ4FGL J0900.2-4608¿ïÿºÄ½Ó¿†* Û[ À:Ž‹µ«HÀ<hõŒßw@a~#òM@'ª\_|g?Ò|Jž‰Ãc?æüÑA¦"}@	âšÛ¸ù?þUºêw,²¿èÌâÑñϼ¿å¿SÒå낿ӷè99Ýq¿åÇ¢'¿î2ÜÌQ¿ïÿ'Þt†UNASNone
?Ë_Óþçð?ÅBL¼ãº?é(F9D?ÅBL¼ãº?Õ3@#äî¯?Ô,vé؟
?åf_î
ˆ©?Ô,vé؟	?Ù}ƹLd?¿19ʯ?ãA£YûÎ?¿19Ê®?ÃÅ÷ŽÅ:ç?¬è
Û"fQ?ë'N±F?¬è
Û"fQ4FGL J0902.5-4727¿ÔJNd4]¿âŒ0êÄ/À9—áZùJÚÀ:Ëu$oK@ =¢wä"@U
`¬B?ÆíÂ;?…Õ£òQ5?ÄøŸ£ô¼U@ÅKSuÙ¿íék¾êáá?ïî5gÀÙz¿èQˆ˜`´¿é5#˜‹| ¿á§a8)<9¿ÛoÑ~ã4îUNASNone1FGL J0902.5-4731c?뗡¸Êš?ÁŸ ›Ы?Á¡zՙ?ÁŸ ›Ы?î~ZÑÈ©2?Â6*2ñ	?¨RãulÑ?Â6*2ñ	?èé«ýa3Ù?¹¯¢«Ê¬?ÌYP
{0œ?¹¯¢«Ê¬?ïÌÊ[û?ÿÕ¼üC?œÆf´Ž@°?ÿÕ¼üC4FGL J0903.5+4057?ÑÂz³ü‰@DÚË}At?À;­RÜEæ"À=û¼¤`@ {åóìÌ?û¾Îø 7®?޼ɴêWø?ÆÂx¡[?íìw¢xæF@â!Üɚ¿ïÿ€H»Ê?ïõæ °Ï–¿ã¡Çe"¿¿Ø»;ÀJˆd¿Ñ5¡l犿ðUNASNone?ïýÖô!H?@85>õÛz?79H^õ¿N?@85>õÛq?ïüÒ¦ÎñK?VŽÔ?z?9jɈu«œ?VŽÔ?z?ïrÕ½Å?‰ĺêÝB?ˆ½ãJŽð?‰ĺêÝF?ïí°e?Rñn$?bOçšïá?Rñn$ƒ4FGL J0904.6+5200¿î²nÈ@D§<`ŸÀ;X*CbÀ<Â?Úác@?o¾Â@ÚCä'?ÊÇãÍ¿¡6rWá=r?Õ[¥BDH@
ûx¹ u?ïõõòðM¿éÑ(| ¿àœúAzÓ¿î›;ùç¿ïÐlÊ-¶?ïÎèӓUNASNone?ïÿÖgT>üöËò¬©>ôÌ9rÖf5>üöËò­{?ïüzõç?i´(¨¬?</€W¶?i´(¨¬?拉õ$Ì?†ˆZò?†Ö'¸öÌç?†ˆZò?ïü97<‡?3_ÞÃ*—«?>6Fǂþ?3_ÞÃ*—©4FGL J0906.1-1011?ëæΣl@7ä=F²køÀ;ÙÙ$ÉäÀ<­¶‡*@üÎí¹Vx@Vçæ-Æã?ÇyåHn¯?¥³Ûd?D¹?àE†6`å?ñ¸'Æ@Á'?ïÿWߣ¿êw?&±p¿á"g¾U:Å¿âvYޘ§+¿æx²™Dà?™ü%]1šUNASNone?ïüü|—>B?: a´è?8F
ïF?: a´è¢?î𯈦?±Ã¦U¾Ñ¤? ÿ•÷u§?±Ã¦U¾Ñ¤?ïÞ(‡6–ö?ròLŒA?pë¼d´…l?ròLŒ<?í+2ðï
?žySjyŸ?¶¦h{‡®?žySjyŸ4FGL J0906.2-5337¿ï÷o{™ÀQÀ"?Åè­À;ƒÉØ)øÀ<žæs.Ì@#XîßFL?ärÈ^þèÿ?ôP|V?ïõJšX{@["UU@ӌ1Q0Ê¿ïþÜêQB?ï˜Ê õîÚ¿ð?ïÿÿ&¦³?êbÙHÜä¿àC ´UNASNone?ïîgÇMeï?h¥fÖÞjç?a˜8²šµ?h¥fÖÞjê?ï﷝[?"QÎ%I÷4?`ìHbü¤Ù?"QÎ%I÷3?îêȀ†Ÿ?˜	tîdz}?¡Swþ–?˜	tîdz}?ïüÜ®Xæ?EWûÅoK?98ϜX?EWûÅoW4FGL J0906.8-2122¿èŸCY¢ç@1.¿üÚ±'À:'ŏÁªÀ<NÐ& û@F»Å™5@ÎC$Aþ¨?Ä°uh·Ïe?ﶰËåF@@Vý<×!?ýÐ$ˆu…¿Øå#»qп±áêìžF¿è×Obîœj™Ñ;¿é>"Õ½6W¿ïk|»<'UNASNone?øFjqª?§k3̂"r?ïƒäæV9?§k3̂"r?}[ùy«É?ŠãŸ§¨9º?ïÅH

̨?ŠãŸ§¨9º?Ò®5éäW?·éÍ6ð(¡?æ¨å
±T?·éÍ6ð(¡?Bäò¼©x"?6" ²ë?ïûFÃPÕ¢?6" ²ë4FGL J0910.1-1816¿ÎöÿkЪÌ@3¿.Y¯ž¿À;)t"&"À<™™'óe@ U'}‹Q?ú€3çŽ3?Õ?¹=ùµ¹?áÒáïsÁ@¦"¦óõ@N·[÷M?îÖì
µÃ¿ïûÉeeà?ï³t'Ü¿¿Ý~ŽÑ¿{¿ïømÏç3€?ïk²ÖuUNASNone?ïÛÿ'?)?xå='έ	?r6àkq˜?xå='έ	?ï˜á¬¶n…?§¢"7!âƒ?‰Ç"Òd^Ý?§¢"7!âƒ?í´tôÛ? ø^üõd'?²\\[ñ)? ø^üõd'?îgÃRpH¥? à#¸ÔÔ
?©ƒÊØûu¬? à#¸ÔÔ
4FGL J0910.9+6055¿ì}èUŽ¨@D:Ü
²À;€Åt÷TÀ<îÈ8–@³Bâþ'?üiÇ)Ý;?Ô¥:´e?Õ¥óD/Ú¹?ÿîãª2n@·7œ¤eû?ïÿÿ^ðP`¿íõGàiaÃ?×de$œía¿ãí:`Nq¿àq9~%õ³¿ðUNASNone?ïþžOæ¤?+[)þ^–"?&•¾'î?+[)þ^–"?ïúÓ¤7y?låüހa¢?D±o"øh?låüހaž?ïNŒ½fKd?Ž0°4'?–.hS6"{?Ž0°4'ƒ?ÜI?wÌÐНî?ˆúíœX?wÌÐНí4FGL J0911.6-4738c?èH'š(Z?ۀWÿ|ÙÀ9
!¯éÀ:ÅËÉdc@O9k²r@V½+o"?Ñ,B]ó{7?θ3b­õ?ú|°Švæç?úr¿¨X¤?ïïwâd¹"¿ÐØ
]5»#¿ìk–@ô'ã¿ç©&¿ÝP(¿é«Þ…_?Šú)"ç8'UNASNone%?áƒN"§º?Ó/³]ºy@?ÜùbØÞ°‹?Ó/³]ºy@?äfBê¤ý?Öõîºÿnþ?×3ñz*¶?Öõîºÿnþ?ÝB—‹Ž>{?¶B¤†l?á^´:8àÃ?¶B¤†m?ÍvŸÑǦô?³uœs?è¢XŽD?³uœs4FGL J0914.5+6845?îÆÉM?ç@BìÖÜGªÀ;ehžOÀ<ñ¼‡Û+4@! XÐ{®?÷#ք³ž?ÙúõÕÒó?Îf!‡+?ó–*C hÁ@Ãà`¨a^¿ã³!ž¶9¿êZ·D¥K¿èts¿ë<ú¿ÑUíýôâë?'Vä#'»»¿ë5tV2UNASNone?ïúû
p'3?@~]£Á†è?DÊ=»0"?@~]£Á†ä?ïýȸrˆr?Q~B3@ø?1º<k¼p.?Q~B3@ô?ïºæß5G}?|‰€W?FH2®!?|‰€U?ïúI¨^õ?>ËîE4?Fہ^",Õ?>ËîE44FGL J0916.9+7756¿ìxö‹'Ð@@åñà'Œ7À;ž«ôÌÀ=
àj8'þ@kg|×@v8äM?ËÝ
▸"¿µô<'x"ç?ækøÉ6@ͯö¨=¿ïyªæÈ÷U?ïý÷²S¤Ã¿å¼\aÕ²ú¿èL¶Ç§ÉÞ¿Ý}°6Ä¿Ð4'cšY2UNASNone?ïäœ:2A"?ptÃØx)Š?kcÅ;lì?ptÃØx)Š?ïö–U2_?x^2lŽ-˜?RÓõU›@°?x^2lŽ-˜?îçHG)C?•zÔ´œ¸{?¡‹{o;Ö?•zÔ´œ¸z?ïØ;IÒôÉ?f%·J?sâ[…›ý?f%·J
4FGL J0917.9-4755?ïB´‹¸š‹?ÀIܘÀ8ôIÐ-ª]À:À4¦Ð¹Á@P'˜÷@#9¾?ǾØWðVë?ÓéÄKd­@èñƒez®@e«…ÕA¿Ô0÷б^¿á§—Sn<¿êœ…ÂL@J¿èà"¿íÁ9¿ì?û}º@¿ïÿ""ÆUNASNone?Ø· ÊNð?Ò¢ªÒNÕ?ã¤/š÷؈?Ò¢ªÒNÕ?¹ÔL½Þ]?Å¥¨¶J"?ìÅvh\ä4?Å¥¨¶J"?Ö~'¸*Ÿ?´è¹·<?äÀì#ê°?´è¹·<?¶!¼"#Xó? Â)¥)†v?í;Èo{"á? Â)¥)†v4FGL J0919.3+6607¿ïþ3ß@C¨ów[0À;$¬þÑ+×À<Ä +"I@ 5cqw'@V#£s7?ËöJŸ‹v?q$Ã-è?Ÿñvû4@ãæé¸l¿èòžm"׿à]àñFÿ™¿è@å¾5ZU¿ÎºE¡ô¿â}a?5¿ÛÂ;yRÒ5UNASNone3FGL J0919.4+6604?ïþó¢
?'oºCßg?/ÀÅßH´?'oºCߏ?ïýØî
°?RPu[ð¦ô?18¯'"Æ?RPu[ð¦ï?ïô×/#/‰?aæ0<½Ó	?VQ¡¹ í'?aæ0<½Ó
?ïø¼•*¨!?=*×ÚÚ	?M
«U_}ƒ?=*×ÚÚ4FGL J0919.5-6203¿Ý`—ûk¿OÀ!tBÇû¬´À;,¥R4€:À<øðž³µ@u†6:y¤?üÅ㤧?Ò
 $Ð?è1³¡'œ'@ü™˜f"@8ªÄbC¿ïþ$}㰔?ïÿ5Ÿôým?ßnD¡o¦×¿Þ!ÂÝà›a¿ïÿ胸›¿ë©ââÔ?UNASNone?Ýc·«BȆ?ÊÕ4nwÎC?áN$*^›½?ÊÕ4nwÎC?ÏNêéVµ?҈fGá"^?è,yÅEªS?҈fGá"^?ϟdãp·?³Ö|€õœ?è&Ç#Ò=?³Ö|€õœ?ĨŒ;aù?«œMÇ=H?êÕÜñ'¼?«œMÇ=H4FGL J0924.1-5202c¿èŒš6¸$¿ój
ÃödÀ9+ú—á2µÀ;#"i†¬@9ñ–°±
@C«»Û
?Ë®™Æe)¥?¿g­Ÿq0*?ôTÿ†]|³?ô(|P]?ïúI<‰ô
¿ã1T?v¿ìˆè6ú¿ãÓW€o|¿ïØjÅp·ù?é°â`‡ÕUNASNone3FGL J0923.8-5154$?îûü'
j?µâ¨ö&Ì? @6î¿Ya?µâ¨ö&Í?êvéÛ?Ð*Fş¬?Æ'ÿ¼X"Í?Ð*Fş¬?ê_"Ôv¯?­èäPñ)¶?ƃt¯²%B?­èäPñ)¶?ÚÅ°{¼‡?ÀÚ})æžÀ?ây§Â!¼?ÀÚ})æžÀ4FGL J0926.1-5336?Û"™WƘÀ蚈¬âÀ:"hZ\lèÀ<P+žê;s@sCC¡•?ûŽ‡Lû‹?ҏ—U»?ç€ISQ·@
ͦ‹ðd@]aXµxÈ¿ïø|}ÿà ?ÁòSD¿À©çÚð&¿×°³Ü»Ø3¿ëþYl'à¿è¡a«ÃUNASNone?ÛÔÔZ[â¾?É  ¯4'Ã?â•ÒÒ¡?É  ¯4'Ã?áv˜XW
[?ÕQ)•_I8?ÝÏOQåK?ÕQ)•_I8?Úuó.ÅNw?¼i$ºÎ—¹?âÅhXÅ?¼i$ºÎ—¹?Ûl"ê©gÉ?·9í¡B†i?âIµŠ«L?·9í¡B†i4FGL J0928.3-2713?ç~gᕈ@0úZxòZ%À;‹n]«­À<nÒæÂAY@ól¶6³E@w³•Ä"?dž<š«? ûéoð©?×=ÐE'Q~@càη]¥¿æLä_:£¿ã;¦i‹´Õ¿çš
¢ñ10¿ï÷Í⠜?ïŽÿªo«¿ïú#|ÜÊqUNASNone?ïÿ=ÐÓɲ?Ÿ™@#§?Eå†É£Ë?Ÿ™@$ ?ïý™0u×w?UùÕK^"?36|QDH?UùÕK^–?ïÛ$2øù?uÀÄæ?rwí惃*?uÀÄæ?ïÿª"3?²6XEy?Zó<9o¿?²6XEyÞ4FGL J0928.4-5256?Êãt)!¤°¿ötmZvnÀ:4^'Ӄ À;²'Œ6ڈ@!ÈÝ:Ùâ@%"ü|?ÝTd0V4¿Yõp7©?¨#¹ P5*@^
›h¿ê·'ƒû£?﹞âƒÃD¿Ü5b¸[ü€¿èìí¼0¿Åօˆ?ª¿Ô¨˜¥}ÓjUNASNone3FGL J0928.3-5255?ïÛþº"§`?p–ò	ð®	?r¢½¬P;?p–ò	ð®?ï²ðG‹~?­´Ý-ã?ƒCþn ±?­´Ý-ã?îœ_Ÿÿ?˜îÄð7[ê?¦:¾?˜îÄð7[ê?Re'%?'LG²æŸ¯?"kf›v´?'LG²æŸ¯4FGL J0928.5+3916?Ú¦…°#8@G:Á~ºñÀ;V›‡À<¼‰íT+Ñ@‹	ˆêË?ùÛR6-¹w?âÃ^YQªí?àyÇQc?õ
US«È@·r0É÷Z¿ë"ÿ*¿äÛibš)¿ØßüTyÕ¿ã|É´êWø¿ëáÂ]B¿ïÿž`¨·DUNASNone?ïõ˜ùՉ?X:"êüË×?TÏTì›?X:"êüË×?ïüøT
ª ?WÇûƒ%RC?8=_'®ÿé?WÇûƒ%RB?î}ÈY
"?™^yí@—X?¨#znï-ß?™^yí@—W?ïë§Yu2œ?UØLR¡"Ö?dX¦ŠÍd±?UØLR¡"Û4FGL J0929.3-4110¿ïô~¾ß£5@Û¼ôèuÀ;¡}‹QÀ<šÐüÝ5Ñ@$œþ0'~?÷´¿û-2h?Òj«ûØ?£bt"Q†0?ÐXÅ>
+ã@džaƒ}£¿ï½ÜÿõÄ?ïÿí@_Á‡¿ÞÚf]­[¿œt‡Äã|ð¿Ý³n!EÊå¿v"쩃iUNASNone?ïÿHiÃÎ?±Ž?òÞ†Mý?±Žg?ïðØqÝ´á?Š)`Ç]'?^OD–<ä?Š)`Ç]"?ïé¿~Ô?o\p·âz?f@o+å¼?o\p·âz?ïà'Âã3?jImÎƛ™?on=Ìêb?jImÎƛ›4FGL J0930.9-3030¿à/GüO@.&?Ýe¡EÀ:àˆÛ—À<z á!¨@ ê
½,ñ¦?ÿ…˜Æ5?ÄPƒO*`¿z¾z~À21?»5y3'K?û1Åû!sî?ÖpÁÊoû¿ä ÜïYÀ¿åk¥€Âù¿ÖÓEA¨–ã¿Þ
`¨6j¿Ó_2•~'UNASNone?ïûJ|?:aÅÃ$P?A¿í¾Ö²?:aÅÃ$\?ï÷ñÞÉ?mÉÄ|z?QÚxœBmð?mÉÄ|z?ïõ^1]ág?XeÖ`Ù÷?UCD=1Õ?XeÖ`Ùé?ﳟ7xð?kR0"ÿã?ƒ2!Ãýú?kR0"ÿã4FGL J0931.4-3559?ïŸ%˜þÛ@&vT´:çÀ:ÉNÀ<\ø_»Q@  x"¦s?ú¿Íui8©?Ô¹CXr?Ò¦:&l{S?÷²åB˜@l©4:D?ïËM;5Á¿æ¾‹@hî¿Ú"Ø\¢î,¿Ýzz…\!¿ÞŒy¦Ž¿íò^ç1UNASNone?ïú€i!-?LÄþuÞ?Eþ[{"H}?LÄþuÞ?ï𲨮"¨?vá|l
¼!?^š®£º±P?vá|l
¼"?ïI¾E/:;?'ÝëÃ?–È7Z¸y?'ÝëÂ?ïž÷s+sá?s.wŒðÝ?ˆB#5#®?s.wŒðÝ4FGL J0933.8-6232?ìB§À÷þÀ¡2CI*ìÀ9þSW•éÀ<;<v¨Ô@­â˜»ù?ùï:µÞt?´=ÜÀ›ø*?æ&õ7O!¦@0M™gD²·?þ뮔¨n?ïçŸìš?¯GW™ˆ'?‡Æ¨½ÆA¿àµ¿äF¼¿îÚpžùÞ¿ïÿȽs"vUNASNone3FGL J0933.9-6232?e¶i¸
Œú?c½‹Hµ~?ïêI–Gõs?c½‹Hµ~?p3•I(Ðé?>à—ÝóB?ïߘÕm®^?>à—ÝóB?¶FÀÚ[¶V?¥×P~×+›?í7'䴉5?¥×P~×+š>žÚM¹±ãT>¢5ˏ!i?ïÿÿ	-'2>¢5ˏ!i4FGL J0934.5+7223?±1–µ&ž@BÏrÅz%À:Ð.ülÎÀ<–'õ@-ÄY`Ä@Œ½}¤p?Âê¹Ç·d0¿¤òåˆZ'?Û·pú¾øy@ûow‡ ¿á†XVÙ+¿æ潤:ÝL¿êžÔ6M™ç¿ê~"àÍ4Ò¿ßÜ»­?¿¿ïNŸË6öUNASNone?ïøð¦|Ó?QaêPW?L?ùf¶
?QaêPR?ïîFGå)B?'™û4#?a¹¸Ö½º?'™û4#?ï'õ5[U?…5‰ÕûE)?‹'²©>êœ?…5‰ÕûE(?ïã©ËÊÕ?`žÈ+þ–¹?lþV45*¢?`žÈ+þ–¶4FGL J0935.5+1152?¹t
_ðÖ@DÝ%þ—J4À;Öß3םáÀ<åCÖïe~@#^m"?ùÈÛ–ª?Ìù)a£3 ?cÕN?lì+@ÞM&yfs¿ïð®ôt±ƒ?ïìÐxR÷õ¿à5A` J¿ÖN0d¡À/¿è2D‹JK~?Õe÷áMRUNASNone?ïý¯_rðç?7xd•à@¶?2…hxÀ?7xd•à@¸?ïüc]B?Z°^Ïâ%'?<åýïì?Z°^Ïâ%"?ï¼Å¸¯ž?'gõ@Üd?€Î'Ô9˜É?'gõ@Üg?ïߟŸÓe?h'ÍÛYÕÊ?p00M|L?h'ÍÛYÕÌ4FGL J0937.6-3358?éÌssúL@+&&ö¶À:Ä"À<6U¸™9"@®É"¾@tþ½	á*?Ãë"ÈÒc?–9;F8YÊ?Ò}y]9!?ýyðql©Ì?ïþ‹ Z›¿çš€'¿í.jÁ¿Ój¿ëíAÄÆn?°äÏÍÞѿɶnçi[8UNASNone?ïóÅ:ÇÞ?bC49p?XuŠpCÍÁ?bC49t?ïÅ_j/K? 3ÚÅ Ä?}PJèZ7ä? 3ÚÅ Ä?ï.j
‰E5?'=V–J_a?š2¾N×YY?'=V–J_c?ïàð^s'?džKPux?oࡌÙI?džKPux4FGL J0938.8+5155?Ã^zË5:@G>L/ƒ{JÀ;Wѹ›—¡À<ãÕçþ{@Å$ʏ°¸?ÿÚáb†?ʨ3PD¼?²z5?ÙJ?éwÇ·º@ã,€±¿å
f H	"¿ä©£1ÈÏè¿å˃á÷Vc¿Ý÷µƒ¯øV¿ÎíŠG?¿ïÿ÷Ò4ÛUNASNone?ïþšÅÁº?&5K}8Á?&S£çäl?&5K}8Ê?ïýœôœ"ø?L•0^?3[èC]?L•0Y?ïô^°ÕýŽ?aµJ'ø¡s?WBžTã?aµJ'ø¡u?ï÷ݜ'–?AÇL"­Ð]?QÒDÆÚÖ°?AÇL"­ÐX4FGL J0940.3-7610¿ïå­ó{+&À1sàGÓÔÀ9Ã(xÅ
¼À<'šÈÙ"@}ðpÀÝ@:a'ÑÖø?½=߉'æL?Øü
Ý©"ã@xØ앿ð@Kœâþ?¡Ë¸$Ê׿ÃÈ{ÄÇoÁ¿Ý1{"54¿æZ—ZúøY¿ïÿëJw¿Ø\:~6UNASNone3FGL J0940.6-7609?œrÊBÐ?}°ŠnºÐ?ïÀÇÅk{?}°ŠnºÐ?§Þ6))Å?µõ¨óSV?î'—-mc?µõ¨óSV?š05üû??äâ+ûy2?ï.þP&?äâ+ûy2?ºª¾‡´]¢?žUlzé?쪨/	tL?žUlzé4FGL J0942.5+7620¿ï\=beWß@Aî‰v5çCÀ;ƒS¾ÃõŽÀ=MŽ(LO@ N
/-êõ?û]þ¸Ø#?Õ$¾!ŽE?ÝN']Šõ'@v?<Uñ¤@Ý]Ü)6/¿ïöK¶··'?ï÷
XH–r¿á³"6‹­H¿Î(ú »¿î™ð×n¿µË4*©øUNASNone?ïçäXo.n?lω®g±Ÿ?h§Ñ'ü?lω®g±›?ïö©/÷?lï&'ìì?Sö­ ø¦?lï&'ìì?î4]K։?œ‰ªı]?¬¶*+B—g?œ‰ªı\?ï%^ãØi?‹ºXÌ{ù'?›]ô#"òÛ?‹ºXÌ{ù&4FGL J0943.6+4207¿ï'ÌF°öz@H"­}|,¡À;"‰"hØ1À<"5¬En@¿KŠíÚ9@H…ªÏL?Ñë¹÷Ýò?¿Y'A'+'?ï|ˆçš®m@—¨q£±K?ïË'`—¿èŒµ( 2¿åš'bEov¿ç,	þÜix¿ïÿÿ)@k*?ï™HÁ9ñ"UNASNone?ïÿŸT-ÿ=?WÕñ~¥?*ô€0‰?WÕñ~¤¤?ïû~Ú:‡?rRUô‹J?B˜—án?rRUô‹I?ïÞyñSþ=?o ¿9»a?pÃVá?o ¿9»`?ïúËDö% ?:ÿ5:
ó?DÒì'k?:ÿ5:
ö4FGL J0944.6+5729?îÉ75AYø@F¹‰ßrïÀ;Õ09ƒ¯MÀ='¹@ ۑ×-xß?ÿœPbîâ¡?Ñè[ôrƒ?'ÅiV/âq?¶¥ŒÁïÏ?ý§gıË?çD ¾{ü%¿ãøÃ*Œ›"¿åϙ/çNX¿Þ§¨ìMñ¿à¡¿}ƒäQ¿Þ73ÞSÝÎUNASNone?ïý@7'1?4æÀ#ÒDã?5þCîwU…?4æÀ#ÒDÍ?ïú‰Û
o?aSÙKèF
?EÛܓÊB7?aSÙKèF?ïõ§­‰?a!$¥2eº?UÞ°¤íç#?a!$¥2e·?ïÑ}aâÁd?cko–z´?wAOŸMª?cko–z²4FGL J0944.7-5124?ë¾÷
vß?övaÍ
àÀ:xÙÔLgÀ<»få@ Ú¤.™p?ý{ÛB±U?ћ)Q2!»?ÏîƒUà\L@S_2•?ý%'6¥®{¿âšÆÀCQŽ?ïÅ2¤—ú]?Òë@Ö3ÿ¿ØîŒÛE5"¿âù́'²Ì¿à¹ë^2eXUNASNone?ï­¥;¼ð?›¢rV'A?ªKXˆb?›¢rV'A?çÙ@œÁWo?ÓêÜÚ¬™?ÐM~Æ}Q$?ÓêÜÚ¬™?ìOÎ¥Az3?¨ï[Ô¾?½ŠÕô.j?¨ï[Ô¾?êº2ŒŒW?¬@eß83ì?Å5ÍΣú?¬@eß83ì4FGL J0947.0-3548¿ß××B™v'@+ˆ7q†UÀ9øúÒ¶À<óähÊÅ@FjpŒ/#@\0LÎå¬?Å=ê†Ç?áÇV +à@ìxc¾ì9@œI1wF^?ï«<ú\R¿à±%q©ˆ¿éñ&³ÈïÈ¿ïÿÿ" 5•?ïʧ߭z¿¦:ÌbLXýUNASNone?ê $±8lØ?È/ÔUÄÿÒ?Çm;L¢?È/ÔUÄÿÒ?ì¿Òó‹?̊f¹÷Ã?ºñhc§q?̊f¹÷Ã?åb¬¼ü/q?¸@Ô§ãé?Õ:¦†¡?¸@Ô§ãé?íü"b´™?°Ô,Y֟?°\ê[7{?°Ô,Y֟4FGL J0947.8-4234?í¨Ó®%-@ þØôù;ÁÀ:[=~HÀ;ý57ð1V@¶ P¢@°cûRV?ËOÿÇ é?Åëq¾cÒ?úÂ(]í@Σ'•¿Û¡ßyw»¿Ã³œd¥-¿å]&¡ª_:¿äÞ?:þ¿éð9¹_2¿ïÿØ}ZÙUNASNone?í}æ $Gò?³QŠ'?´ÊþÝÀw?³QŠ'?ïšW5o?¤Ð$½}äØ?‰j2¼d;?¤Ð$½}äØ?í•ìF1î?ªæˆ:ÀÔÿ?·cPÎp?ªæˆ:ÀÔÿ?ï@e¤ú]?€‹J·/?—ó_ë`´X?€‹J·/4FGL J0948.0-3859¿ÓüŒ,ÀË @&y*Qã!£À:¶¾(Å(À<£hOt²@›"j8-@A³ÿvmE?ג¥^žÆÕ?êÅÂíOú@'ë¾íç?þ õ;5?ç÷X[á¨&¿ÝñÆ@ì"M¿ìþ£^"_ô¿ïÿ'ãñ?ïø¼ßï¿@¿ïûÂ-·sUNASNone?íN‹@z?»Ì\\á6?·m‹¥ÿd1?»Ì\\á6?èH8'©
"?Òs2¶öÛ?Îßa[Éð?Òs2¶öÛ?ã­bTq¢ã?·mFåÙì?Ø¥;Wº9?·mFåÙí?ëØOò<´?¾
Š{§p¢?ÀžÀ5û
2?¾
Š{§p¢4FGL J0949.8+7551¿î61yH/)@B?ÖbwÄ]À:îJÔ9¨˜À<ÚµŠè@ø™Iè^?ÿj~…A?έ©MÙ?Ó¦¿òɶ˜@¡/à˜[¬@‹¸Þ6¿ë¸Á>#Q¿ÉÿÓµI¿àÃ.ô	Q¸¿ä ¶© ¿èae`,¨¿ïÿõƒ¥;ŽUNASNone3FGL J0950.4+7550?ïÕ§3pÂ??}*ßSH>¶?u,fGžà0?}*ßSH>¸?ïñT=ýLh?ye+%êKx?]W"g0?ye+%êKx?ìðʸz6?¥U¨Á¹U?¸áª<.M?¥U¨Á¹U?îˀ$BU?‹Ÿ ŠØŽ—?£Gý¿›Ú°?‹Ÿ ŠØŽ—4FGL J0951.8-3711¿éØ?ìÁc@*-À3aVÀ:µž·æ‹»À<:îí‰@AÜ¢òô@¯BÇ$í?Ö9íAat9?î~;¹ÿk@>l`{jÚ@3ô–#î¿ìÏj¡^‰ù?¢Âæo
Nã¿ìà=lòò¿çí?3¶?¿ïüBK?ïęAÚëÉUNASNone2FGL J0952.7-3717?æ«Á1§‹?ͱ¾Þ?Óô¨}œ°é?ͱ¾ß?൸—V(?ԅÓÚr7B?ß̔ŽÑS°?ԅÓÚr7B?ãJb¾Uj?·YØ_4	?Ùk:ƒ÷U)?·YØ_4	?áޅð#+¦?Â$Düyæ]?ÜBô¹¨µ?Â$Düyæ]4FGL J0953.6-1509?ê×I"·¿V@=šO—íÇïÀ9Î,UÉ`1À<ˆ¢Ù´;Ü@"²U}5
?ú»	 :2+?ºžolIP?å(U{\˜@%%"1zÌ@9RIMü¸¿í<Lû[V?æžÞ&'d¿ÉMgfìs¿æ	s˜Ôx¿î"žã…uö¿ïûÌßÂðUNASNone3FGL J0953.7-1510?tN†)ÎR?ŸfˆF'?ï×bó­üb?ŸfˆF'?ƒŽ[Æøç?†ùýšd ?ï±Æ" ä?†ùýšd!?™íÃƍ?'é"];‹?ï7à'çIÍ?'é"];‹?2½žC:ÇÇ?(æóô¡I?ïý¨L7˜§?(æóô¡I4FGL J0955.8-4106?ép ¾WFú@%ì|•|ÔÀ:@\78{rÀ;¼$·om@ÙÜ»W@z[ñ?ÑsÓÜí?â*8ÅC@Þ¦c¬wÃ@]!)ÆM¿Õ§ÕÜëÓοàøi"®U¾¿êû/—@ú¿ïÿò(¦è7?Ѩ©ï?çjNRsjUNASNone?ïã)á=ø?¥Ï0¿u}?£šÃØA
?¥Ï0¿u}?ì/ž'|ÊV?Êg³ü&¼?¾ƒt­V?Êg³ü&¼?èØK8C@ù?²X•?G$?̞Óòü?²X•?G%?ïúr©z}?š=:f?œ ±ªÐ°f?š=:f4FGL J0957.3-3851?ëóÏw;å@(ú˧2ßPÀ:sö•3À;í┵.K@¬Þ½e&@—s\.Ë?Ñ+^×{Ò?Ó
©`áí?ü%F
¦L?ö—‰çtî¿¿ÞqOÎtm¿ä[Ò>%Õ}¿í»ñ³6"Ò¿â'¢;(Êú¿î»Oag#%¿ïÞú̺XVUNASNone?êCîÑæ]S?Æ
o\љ?ÆðD¸fŠ´?Æ
o\љ?ãÈÿöi‡?Óñÿà=?ØnÖ,ñ?Óñÿà=?åcÅ©<¨K?ºŒDæôƒ?Õ8t­†¯h?ºŒDæôƒ?ß»X†;Á?ºŒ0ù"Éä?à"S¼âu?ºŒ0ù"Éä4FGL J0957.6-3051?ì6Þã¯bÔ@2µ,'¦77À;(Òü'¶vÀ<šˆÉg½~@nןc³@9lÅûø4?ցùje?ì)KRä©b@
´¡\Üyé@re"C¡À¿æR:Ê×)G¿Ö™}j¿æt5ýö¿ïû©žõN ?éŸ@¤Šä?çÂ)óUNASNone?êä_¶8
?Âíçµðf?Än'—×?Âíçµðf?ë){	&'p?ϱڂL$?ÃZÛeºB?ϱڂL$?á·¦žNõÍ?¹œ–ÙÝ=?ܐ²Ãbd?¹œ–ÙÝ=?îpÒN?ü¦?«5I»Ïjé?¨òÛ5¬?«5I»Ïjé4FGL J0957.6-5208?²ÑÇQv@ɤ^ïÀ:€<_+߂À;Ï _Š@è°XÍÌ|@X¢t3¯?Êm§"n>ø?±´p	¨Ja?æͳaÁ»ø@Xœsé†Â¿î;Ɵâ?ïöÌD琝¿áãñâ0a¿é+ñUBQ´¿å"†ŸìÄå¿à—|ÞÍÖ7UNASNone?ïðóDS?`0í»%ÈA?^wÃYÈ)?`0í»%È??ï¶+;hB?©Ú‰÷mº?'u1%ï\è?©Ú‰÷mº?ïg|?•£ùvÿ?3üPF?•£ùvÿ?ïáÂÎÖÁÑ?`n¯ÄÆR?n=1)>/?`n¯ÄÆR4FGL J0957.7-3510¿ïá_¢)'@.Οð˯–À:svð!fÀ<(˯–[!@Rqé&t´@!Mryš ?×Ëq'úä?áƧ"=çÂ@	o!öÊÍ?ÿÅäÆh¯—?ïú²]à°Ú¿æˆ(Øîn¿êædþ²M¿ï†Ä);
?æûÎRÞÊ¿¹ŒÔ_":UNASNone?ï¿ÀGQ?"7Ǖ",?€ùî+¹?"7Ǖ",?çñúwÙ?Ò{:÷t'?Ðü
ßN?Ò{:÷t'?æ×à-ÞGb?·©Ý/9…Ø?ÒP?¤Cq;?·©Ý/9…Ø?ì'å=L""?»nð¨ÏE?¾ÀÖžë^?»nð¨ÏE4FGL J0958.6-0522?æ, sšçò@BŒ>§¼À;"žõ#-,À<›w3=D.@ØZ°O¾"@²¾‰¬½?Â9q{BkŠ¿±"Žg·IX?í1išÐ?ù͙Ëî€|?Åû`ž{U·¿â;}^ûc
¿ìúþ£ßm¹?ÙÈuO7u¸¿â¥ýzïð8w?Ò~UNASNone?ïêåtÁ&p?bwëÆßŏ?e‹>ُù?bwëÆßō?ïÀA‡ñ?£'÷6¬tï?ó_<r‡Ý?£'÷6¬tï?ïÍÌÎHcF?|9k'3‡?y˜ÛÎ]˜?|9k'3?ï"	ÍH‹)?'›hœ7ö?ŽýŒ­Ý5º?'›hœ7ö4FGL J0959.1-6441¿ïâœUºÀâDÀú0³À:˜8±ø50À<§÷*ni@Á¥"Ò@-IÿþR?Ðô«£‡Y%?Î"øþYà?ý·}°/@¹‡!m¿Ývz"ð¿ç—ØÏ9Ž—¿çW\¨w'î¿ÞГásÍØ¿ïÿýF\I¿ïƒY¡\ºUNASNone?ïʏ?Qä?{¹á›ßVÃ?zð¸`W
Ê?{¹á›ßVÆ?ïÀ¾ŒBðw? bÙåՕ? ¹Þ‡ÄÅ? bÙåՕ?ì¬.Ýû±W?¨"Ú*` ?ºž‰"uJ?¨"Ú*`¡?ïMqõæ?ƒB¦°7AÄ?–QÝAC=N?ƒB¦°7AÄ4FGL J0959.1+5719?ÕßÆc&ãÒ@G¥"À%À;b,µj°À<"φ»p"@‡Ž6¼@ÂzÞÃo?Ã)2(q8R¿¶ï.vŠ÷?ô`­¤éXõ@6á¿Î¼?ÁqËýTª¿êB±(+˜¿çc˜UÌ»¿ëõÖEòR˜?ØÓ P—ó¿ïþ±¶ÆÑ
UNASNone?ïë`vòÕ?g7t€?dŸ‰ô
+w?g7t€?ïünDã}B?``¼ ).š?<Øäó¯?``¼ ).™?RÁ˜"?‡¥ásC'ö?Œš+O™ÞÝ?‡¥ásC'ô?ïôx"êÃ#?Ru^åvµ?Wº*y¹–?Ru^åv³4FGL J1001.3-2040?ſtPµž2@:ê7&úÆÀ;LÇ+£ùÀ<½oe©P@ ŠUŽ¡™?õL«	-¦+?áÀá?µ"?ã…ߨq£±@tœŠâ?ôÜþ(º¿ëì&ďç?ÐݧESÇ'?ïÅTӖëi¿¸ÜÐ{)Ñ¿æ—IÈ î"¿ïÿÿ" 5•UNASNone?ïì\,
ʱ?nmn‹¬$?c£Óò5N"?nmn‹¬"?îyÀÒ«n?»Ù«Q'~?¨còÞ%I%?»Ù«Q'~?îúÚ©þ.?•\¥¥UCi? _U`?•\¥¥UCj?ç`-]Ž©ù?¹4²'6y?Ñ?¥Dâ¬?¹4²'6y4FGL J1002.3-2810?ëŸ\£®Z@5k»ƒÏ,ùÀ:әt°¬À<<íÜçÍ@n݃S\@!]³9}Ð?çÓÌ@
>?íU/<-­¸@¦ó|cþ­?ó-ƒ«ñŠò?ïö%÷
ø¿ß¸ç¨eÝ¿ìuL}‡\¿áó{jª¿ï÷dP±¿ïüK_ÏÉVUNASNone3FGL J1002.0-2837?í¶ò
?Ã$jÆz{?·:Ho¬×?Ã$jÆz{?Ê
3ÔÝß?Ñ kîЖ?é|³
ùˆˆ?Ñ kîЖ?ç•þ}Az?°š"4žp?ÐÕè}?°š"4žp?[e(á@??Yiå,²>?ïòMk_þ?Yiå,²>4FGL J1003.7+7049?½½úýSºÓ@D4cŠ	À;Ä5LèæßÀ<ÝrÐ×ôH@ ñc='Ó@
&ˆó?ÄÐR¾=èÄ¿·é¥´¦?퉎;Tj@³sŠfK¿åV'""F¿ç5:	Iú¿çú+	™ö¿êø¥˜«]?ÊÃgÉ<õT¿à•½ÀƒUNASNone?ïønóäL?LïêӛàÕ?ND3œnÏ?LïêӛàÄ?ïýöÿÐS?GÈ
«0˜?0H}gÑæ?GÈ
«0‰?ï׸0[(b?yϐ˜s£Û?t#çÒkÎu?yϐ˜s£Û?ïú\¾e?B†à²þv?Fk"¹»?B†à²þv4FGL J1004.6-5215¿èê(ï-p@5+Z÷[À;"÷8±!vÀ<‰E=÷²T@î­94?ÿ÷i=±;w?×RaA
'c?éÚÝfx@¥ߙX@|´>
§¤¿ä9Œ~($?ïøٛhÞ¿Ô¹+ºîÓÞ¿Ýq׳°œ¿ïÖèå1G¡¿ïWîÕSUNASNone3FGL J1003.7-5215?åd`¾Ë•9?Æ¥{À4øQ?Õ7>'hՎ?Æ¥{À4øQ?Ò0d¨+4?ÔAÁþ,{l?æç¹M«êf?ÔAÁþ,{l?æ2moÚ\Í?¹R#5²e?ӛ% KFe?¹R#5²e?ÛÿÀ <-?¸Â–C} O?âïøáé?¸Â–C} O4FGL J1004.8-5250¿î?Ãî[¶@—a_–iÀ;9
ÏÌ[ŽÀ<X·Q:…@$Þ.ŒÛE6?ø†Ì7{—P?Ňϗ­[B¿·¸ËŸ6wÇ?ù¡cýÖZ@JÒ1e©¿ïÿ˜f"²Ð?ïÿõ^'¿¸œmŒ?¿éf è¿äj&¯—1à?Ê[å™w_ÞUNASNone?ïþ®Ü¥±?0˜06‹|?%â5¤ëÏ?0˜06‹q?íÈԆ{¥?Çf¢ÂkG?±¹[Ì"×'?Çf¢ÂkG?ïD¹œÔ™8?"%m—áøv?—hÌelØô?"%m—áøw?ï‹bHË?ŸgÃ}ª€{?žn"½Öæš?ŸgÃ}ª€|4FGL J1005.5-5708c?äTÂÅíô¿ór˜Ù€9vÀ8ùáy,;ÈÀ:s™LlÀ@<½J£½@7­eÿ8Z?Ê»˜Ý\#?ã·¦±.@ö£ð4±@ðbF¿íÖ®b~zY?é0ðÎ3Õ¿çñûûŽ8¿ìài·ª¿ïþ݋`ñ²¿ãÙ}'ÕUNASNone,?³Eù)¡?ºnPˆ*Š?íž7@Úތ?ºnPˆ*‰?°uÛ
œ?*)Ñö&?íðQDžM?*)Ñö'?Æ7?'Þn ?°úÌ1+Ǘ?êr0ˆdX?°úÌ1+ǖ?{3"›Ùß'?j.s½Ÿ?ïɘÖÈLB?j.s½ž4FGL J1006.9-2806?îѯ§õëv@6!>‰¨‹À;=Õ¾
iÀ<m7Žâ†r@ÅñÞ&Ò@™þ†ƒ<`?Ì™<§{/?'ÑŠægAq?̃ÛÂ3@‹µ`£¯?ïåe¶™…?ì†e	o‹¿ì£é~´;¿Ø%}}":7¿Üøe-×)¿ïþ´ -UNASNone?ïࣻ}£?s"›)îï?oë\D'\J?s"›)îî?ïÕU­YL?"ç&.£9Ð?uU|)SYð?"ç&.£9Ï?ïRd8Æö}?'ƒo¶Ì^õ?•³xç!0_?'ƒo¶Ì^ô?ï™Zã("¨?yNB_€ž?‰©G5÷V
?yNB_€ž4FGL J1007.8-4514?ΞÅċ¥Ä@!>—Ðk½¾À;^(Àª'À<p‹â÷±}@!ö¤Q-š?þù²©5?ÆÛK•ª¡ª¿²ˆœFG7!?óõ«é'v@vä;ÿ4©¿Ó¬ž"Í¿áw™:¿ê®ßa$F¿ïÏüE±?îüwµCCL¿ÒP|VUNASNone?ïþ'¶£yî?,2J>'ö•?&ԕÈa(?,2J>'öã?ïû0æW¨t?gRð¬H?C<f¡^.ç?gRð¬J?ïž`±r0S?†4xõû™?ˆgÓ£sër?†4xõû˜?ïü£_NÐ$??À¥O?:å‰~åÏ??À¥_4FGL J1008.2-1000?åzñÙ@AߥÁƍÀ:7äÞ;ŠÀ<PP¿54•@ãá5E@)ªIë?Ãb'Z/÷??µvÄ­n§?ëýdQµ@gõ†Tmk¿Ø³D›:ƒŠ¿èfœK›à¿í|KÀrÌP¿åï`«;'¿ï÷¶O²Å»¿îʇB'UNASNone?ïçÐ+ޅI?q¥*§âø?h/Ô!z·¬?q¥*§âø?ïz°*$?¢,Æ¿˜ât?©ýš¼›ƒ?¢,Æ¿˜âs?ï\=B2?1ÀPãº?"xO×¼Ñ?1ÀPãº!?ï?ÛW3S˜?Š{N8ˆ?˜••?Š{N8ˆ4FGL J1009.5-0034¿ï.­GÐJ@Eß;dZÀ; ¯7'À<ˆ©í¤³©@Þ@ÌùÃP@RpEy‹?ÔÅ$'n|?Ô­ÎÚÄU?û¦y–ÄÓ@
›Ž¹¿ïÿŸ‡ð#ê?ïõ}€3l¿Ý ó*.§³¿ç¦Æþ¬˜Ð¿ãmZ@¾61¿íÚï9ßßUNASNone?-çN¹?…?ÅÑJy?‡W´†,QÌ?…?ÅÑJx?ïåž;;¦?"ˆ]ÉTN?jaæÄÄ[?"ˆ]ÉTN?íÎÜM8š? UfZß,?±‰—†;/? UfZß,?íå~ê^?›aì܎8\?°Ó‡Ì­?›aì܎8]4FGL J1010.0+1416¿ìPÚÁH<U@I*û~ÿ—À:ëG‰+MÀ<eÝãu…¾@¬¸§{Úl@L®ì?Á¸#G'Ëw¿»wۃÉΖ?ø†!Ðý?ö…ÓÉÁ)«?éÛÁÝ/›¿èî÷ßËF¿íŽÌKD¿Ç³A¶X¿Ñ(}ãǐ¿ïÿ^º z^UNASNone?ï埚1ÃÑ?tVy¨ˆ,?j`eÎ</'?tVy¨ˆ-?ïN0'×ü?²¢"§¤e?ŸÖ9û'?²¢"§¤e?îêb@;$N?˜@&,)œ%?¡YÛüM».?˜@&,)œ%?©à6g? Sɚ(Â?¤5aü™'? Sɚ(Â4FGL J1011.4-5729c?ïýÁìøÞG¿ð¡ÒM?MôÀ8ÁÚWÏÊ®À:Fá$r¦@kŸ~Šõg@b¡ Ï?͹§@¡/æ?ÖK2»"@÷ñsuB¢@|{ðȀ?ÛªcÇOµ?ÈTZŠ»x¿ç½¾a¥"¿é¿*þ~ð¿ïò-DéN?îK®UNASNone,?Ør_ífCÐ?Ðh‰miáv?ãÆÐ	LÞ?Ðh‰miáv?ÚY†/§úç?ÕLܬ¢¼Ð?âÓ<è,‹?ÕLܬ¢¼Ð?ÑÁɏdÁ"?¶@8Éé?ç8MŸo?¶@8Éé?½–û ôï?°¡˜H|˜Á?ìM ›áb?°¡˜H|˜Á4FGL J1014.6+6126¿¤ëŽðÍԝ@Gsý'w>%À<#§ÝÿúøÀ=k-àãÛ@Ãf0‹Ž@'9¾g¯<?Þ:Gĺ¯"?æ"äÁ5>ü@	~?íëÑT›ä¿ïO±^p‡?ï·l]¡E࿺;ùÖEF†¿åèQ'¿è&ch¿ðUNASNone?é»û)m¹o?˔ws^%f?ÉZIH?˔ws^%f?ٖT¢>p/?ÖÔ§üHtW?ã4Õ®àÇç?ÖÔ§üHtW?åÊ+ÙÀÁ?´$üšŽ?Ôk¨L~}Ï?´$üšŽ?˜ŠOÓ21?'Ø%'ã'd?ï;¯Ífo?'Ø%'ã'd4FGL J1015.1-6353¿åP4´~hÀ.ÝÎ|Ð5À:yªÜ·ü[À<(íA°¤@z¤®Ë"ù?üü|¢èÍ´?ÓTª|?ì?Ü9ïô8@—€)†?ú}YÊ¡¤U¿Ô(ðd+£¿äõiøØÄ¿àä›ök+È¿ß,qãr*À¿ç'vµiù¿ïþÎÝHEUNASNone?ßü?¦Üyj}?¦µ¿â6?¦Üyj}‹?ìÎîõi9?Ä~˜UÎ:?¹ˆˆW,¶5?Ä~˜UÎ:?éœTY
Z?±©4l$8?Ɏ®›×Ι?±©4l$8?èT-
ǐö?¯YÊ©;/?ίKÈá¼(?¯YÊ©;/4FGL J1015.5-6030¿àÈCë@CGÀ	¾±›îÞpÀ8¼o´ëÀ;{'¾Šë@ÁIÿþR@Ž¼g#ü?¹µ¥ÿ-?ÄÂÇû¬´)@¨É¸EV?ö`õ˜ó×S¿ÁO¿Ez³z¿ã'Ž½É¿êw$>£©¾¿ëèU{\˜¿àÑÉ oâ¿è½Êeê?¤UNASNone3FGL J1016.5-6034?æ'hO¹Ò?Ë]I|?ÓÜû/`Œ\?Ë]I|?áÿ(å$d?Õ'jüvØ®?ܯÜ5·5?Õ'jüvØ­?䂃yß®ö?µ:¹èF]?Öúù@¢?µ:¹èF]?ĚDÓ/X{?±çp‹öö?êÙnË4)à?±çp‹öö4FGL J1016.1-4247?¥íÆrº°ì@&ùþɟãÀ:H¿è+ÎÀ<L 鄓x@ °æãÏGÑ?ûtyŸ(NÔ?ÂNÔ8üËÃ?Ä+S?î¦@—ԝ{¦@&ÎEÃö?æúÂG¸¦¿ê1s	â×Ñ?æ±x7I¿ÛX'}ÆV¿Ö8\½Æ¿å@W©4APUNASNone3FGL J1016.6-4244?ï«3V¯âb?ƒ¾Wfà E?…3*TgE?ƒ¾Wfà F?ïßÚ-rûá?ºÊ§Ùӄ?péF'º?ºÊ§Ùӄ?ï5òI¶·µ?"}bÂG?™A¶É)	i?"}bÂH?ï%"• Å?‰ 1Ãþ­?›_mKçV?‰ 1Ãþ­4FGL J1016.2-5729c?ëìõVKP"¿åًâvØ$À9[ãU¥NÀ:iÀ¬-@:šœxò@?ޚTª|?È<¨èA€?·6ј–?ò¸ ?¦=@í±GC¿ïø§¡o%þ?ïïNlta¿çU%`â˜ç¿æÓ{rg%©¿æÕ²^·po¿é¯?¨¢UNASNone8?äÇôÿ™@N?Ò£'64?ÖpÍf?Ò£'64?æCªW·þK?ÕçcHå4®?Óx«Pl?ÕçcHå4¯?á$1}?Ĺïùˆ?Ü Àƒ·?Ĺïùˆ?ë
'ía…ö?³HP?Ã×`Jyè)?³HP4FGL J1017.4+5956?ïáMˆ	¢@HQüLYÀ;¥
ÒÁÙÀ=
GR¤è'@¡Y¢<U@´'òÜ+?É -à
?˜K­A[õ?ÐG¯Áú
ó@a+´ä¤?éuv¿ê–ºö6¿Øv'•p?¿èi?Ñ&N¿î)gØVmË?éÒܱF^‰UNASNone?ïñtUÄÃ?_X¶¿g*¢?]TvyÈ?_X¶¿g*©?ïüWûì÷å?\˜wŸ‡žÉ?=@ ˜@Җ?\˜wŸ‡žÉ?ï^[‰Ê×â?I ±L?"4ŽÆ¥Í?I ±L?ïäÛ"Œ?^¿¢þ?j?k$îlsåT?^¿¢þ?e4FGL J1018.1-4051¿æ"V³_5@*"4çhZÀ:¢ï	7·&À<;EM*Ë@I'VT'@E®æ1ø¡?˂ºZ•?ÍÔ`)‹i«?ÿñõ*¹çî@ØÌàBö?îH`A]ò¿ätcI{t¿ç‡§ßW"æ¿èa3¡˜¶¿êÐ0Áhë¿ïÿØÝý ÓUNASNone?î¨êΡû?¦'Ië‹;?¥qSàO9?¦'Ië‹:?îqq0Ò1?·!ìºò ?¨ïìòÜç?·!ìºò ?ìU|""b?©›Y\h.4?½TÛ۔è?©›Y\h.4?îÑKC?'¹SAó?®âî[NkÕ?'¹SAó4FGL J1018.1-2705¿Â…âÚ¾ÓW@8u#Ä*fÜÀ:hõZŠÀ<8a|ÚQ@ɓ¨=÷1@˜ºvˆó?ĪՁ&[4?Á½¿~/°È?ú¡Üär@!͕I¨À?ïý:óñÔÄ¿åvv½Ì¿çmâ0·-¿éŸÚÚ®7¿ä:ˆA'O¿ïúp &'UNASNone?ï'fÔ3—®?"ÂËÊxÛ?fJó·?"ÂËÊxÜ?ï²ç{•á?—pA^Úý?ƒF!¿Gq?—pA^Úý?îÔ|BA!'?šB!¬œÔ?¢¸;Ûíæå?šB!¬œÔŽ?î…zيñÖ?8½Ü8Ïò?§¨RgPâ¡?8½Ü8Ïò4FGL J1018.2+0145¿ã°/žÚí@F³jçÕfÏÀ;$©Á/À<±²•"@]ï-õ±?þŸô╋î?ٔ"â-1<?ïýwå?@dÞÁÁÖÐ?úØ]å
‹Y?ëÿDïY­¿ç˜>»&²¿Ê7Üæ"¿ê'äÏ"£¿ïý!(n´?ïòH¢0AUNASNone?îo^ݙœ?ªôáWn&8?©
&f??ªôáWn&8?ß°Óû?ÖÊå.Ÿêt?à@'òr?ÖÊå.Ÿêt?ê3õ}íÕ}?­¹ÂUð??Ç0*Hª?­¹ÂUð??Ë	?£¨?»3‰$6"?é>½°ß?»3‰$6"4FGL J1018.3-0703?ÑfùIüÜ@CÌÅûø3ƒÀ:¥·gà¹êÀ<c@ìF@@\ mf@"V^±f??Ðyu'
5ô?ǟxÖ«rà?÷‰÷/væ@­9ó–»?炙›L!A¿å)
`EË¿ß
œ¦"Sß¿ïÌdAÈø,?ãèߢ'fŸ¿ïýŒó˜épUNASNone?ïðÞOƒ? /S0u)½?^C`øÅÅÆ? /S0u)½?ïýW¾;…§?M[È?¼Ó?5B#ÒÄ­?M[È?¼å?îéw]>éI?•&ÛV3:'?¡hŠ,kr?•&ÛV3:?ïôä£Y­?SAëwN¹Í?V6¹L¥ÏÍ?SAëwN¹É4FGL J1018.4+2210?ÜRYèW@Kƒ9Ÿ]þ¹À<jQÎ_À=[Ëñr@%+¶ü?ñ¥"}c?çd#Ë·#?ã,ù'þtæ?õáÄüó0?þD!!㪊¿îëç?ï2Ôy±¿îéDg8~¿ïš|¨"2?ïÙ|s%'?À"v>öŠáUNASNone?ïóàí'µ?d?x"ªr?X>%Âږ?d?x"ªt?ï˸jc~ì?§ÔÄô˜
N?z#ÊÎ@Š?§ÔÄô˜
N?íáÿÇí))?Ÿ}~¥>%ó?°ðÀ–¶º?Ÿ}~¥>%ô?溺•ÌcP?"NL¥#ç?†ڌç+ö?"NL¥#æ4FGL J1019.3+5625¿Ü"HoH
@I
¿cíÀ<©.bÀ=5óþj@!
"´ÛŒ?÷ÚWdjã¤?ÝEÈa-A'?àt†_U% @)!ÌÙb@ÊO*Š˜¿àÜäÝdʅ¿ïýE¥ü~k?ï¸7îƒ×¿ÑÏÜâ¹_¿âA¿Þ&çJ¿ï·a–5UNASNone?ïúˆÂNX?FÒ[j‰q?EßÜöƟ/?FÒ[j‰n?ïü=ãZü?fãQ•G0@?>çÝ( B?fãQ•G0=?ï²M˜_¶{?…]µ;"ü?ƒl™èaN?…]µ;"ý?ïèA±Eu?Y€az?g¾NºŠò?Y€az4FGL J1020.4-5314?ν`[@	•,ß?–À:Ž¸c­OÀ<Jr&Ü
@âhgs@½ºŠ&_?Îÿ*˜>?â_t¤íŠ²@)M<É´ê?þhà;"€«¿ïÿÞý¦ßR?ïÿÞý¦ßR¿Ú)ÜÈBy¿éˆÛÜ4I¿én"‡êD­¿ïóóí£*UNASNone?›£îéâTu?£ÖçUTÚ´?ï"àˆ°í\?£ÖçUTÚ´?•àæå?§º1Ç(éÙ?ïPøËx×'?§º1Ç(éÙ?ÃüY yˆ?¬¿ÆÆt}?ëà)—áž?¬¿ÆÆt|?"— yÀ×?Æ_gD¥?ï[Fü3ñú?Æ_gD¥4FGL J1021.8-6308¿ßW@À}VlôÀ;+Ò/]À<'Ÿu{­ @!P-"áô§@¢>ü•u?Ä7A"Z¿³bÎ~€?óÔ*tGÐy?÷Ûb¯L´9?éJZÌÕ0I¿åÈÂ&*·¿è|"Ý¿äå¶rî4&¿ãžÅý0B? ý#à7–UNASNone?ïõ(Iƒg?TgCÐ~?U¯lù1õ"?TgCÐ~?ïM
h9e#?­½ayÝj?–^²øÓ[¨?­½ayÝj?ﺗó+6q?#%¹4??Z52c¾?#%¹4??íøÏ/â—Á?ž#v½}?°9†€ëAô?ž#v½}4FGL J1026.2-5731¿·GÇãþW6?–Òi!ŠFôÀ9éû±¼¦À;olŸe‹@Jê½£@|<âž4?Ŗ•BÇк?æ¢~ù˜@±À"š^»@qܗð÷ú¿Þž±{¸ˆ¿é֑Ýµñ¿¾Nx^
¢E¿ç±×JÕ¿í%óìÌG¿ïÿÚÁ,/´UNASNone3FGL J1026.2-5730?Œ3Š­ýw?Áÿ@wÐÒñ?ïžcª?Áÿ@wÐÒñ?…¹44¶=?•ù¡ñÄÐ?ï©/Ó-(?•ù¡ñÄÐ?²GurRV?©ƒl¶6v¦?í·Qµµ=?©ƒl¶6v¦?he²;Ì{?V	npÐC^?ïçšâMÄ3?V	npÐC^4FGL J1027.4-6324?Å	3NõÏ·À'…‹Å›€À;¬7æ÷~À<š¿£ï]ñ@$»D;Îã?öœY~÷W?Ñ^˜¼¤áv?§C.d'®?Ó5ëŸJÞv@Ta#0†±¿ï†'_8u?äv†ºŸ¤¿ìÏ¡}éÑ?Ûq¸ß¯þ`¿á^@'—FÙ?›"£Q
AUNASNone?ïÿURŸ1Z?ê«=T{N?U¬ÔÊ:?ê«=T{·?ïö˜¢Šð}?‹rp '×?Rκêi?‹rp '×?ïÛÉêf?v
�rp
òL›?v
î˜?ïø¥Ž‰?Mvv(嬯?MiÅ¿Ø¤?Mvv(嬼4FGL J1028.1-3550¿íLÉ*,C/@2‰)ˆ†À;;$ŲÀ<qÀã/@àåK@ðO‹XŽ?ÀŒDœg)Z¿²ˆLj;Ýý?õ$#–=â@t#I†0Ü?ïÿ¯þ_ìпïmªÈ–g?Ò×#gäè¿îx™¿YFÃ?Ò£ƒþ&â¿ÀU\ã°¿UNASNone?ïý<9º?@¨s›_6Ù?6×v20¿?@¨s›_6×?ïùL7Ÿ?oý7؜ºb?JÏ!ƒÓƆ?oý7؜ºb?ï[N:˜Ò"?Ž ÑÎ	Ú?"–8¬å¯ƒ?Ž ÑÎ	Ù?ïêÌQ"}?bÝfšÕ"@?e3®{'óé?bÝfšÕ"=4FGL J1028.4-1539¿Ú=ëòñ@Au~ºñ6À;úÀoÇÀ<vc¹ã»ý@ˆ<[Ðá/@À_@˜?ÎYßð@¿¨0ïáú±b?èu ޜØé@'
_Ä¿è!¡ÇåÝ¿ÎôK@ññ¿ì(Àéi¼¿"¿¹úô9¿çoP…S'x¿ÝݖH¬AUNASNone?ïó1ÊíÆ?V!æÁCœj?Yœäj$sÝ?V!æÁCœi?ïý…˜9Œž?SÞyû~ªÆ?3Ó>3›?SÞyû~ªË?ïÓ¬À|'ô?yU¹"ã>?v)ŸÁìA?yU¹"ã??ïòlp6"è?Mí¾°­œ?[''ö.Š?Mí¾°­"4FGL J1029.4-0828¿êyßo_òø@D@ۜsh­À;!KeY -À<ŽL%r€P@6;ƒd@á#=ò©Ö?¿Ïq—ÇÝO¿·Ž†@ ?õ»‡*+M@ÅCýÛ¸x¿ì!E_…¡•¿ã2¸ÿ»a•¿âc×dÖC¿á@÷A¿á¿¾¥пÄO1ÁnìUNASNone?ïö""?KÎT~â]?RäÙÀ÷Æo?KÎT~âX?ïý[=ˆ?Vzï¥kë?7%&[¼Ì?Vzï¥kç?ïêðUgV^?ríÈ"½?eª˜©¡ò?ríÈ"¸?ï꣞7?T°‰¹Ž€?e=\aàÉE?T°‰¹Ž4FGL J1029.9+7335¿ïŠ4ûpG®@Cü¥aMø±À;–|tÅ¥À<ö)¢¹ @ §N}ça?úÌ
Jݐ?ß.M»tµµ?Õÿ™¾, ó?üLØç&?ûÏ?Ž
oE?ïû³ûð¿ì\šP}F¿áÃ9¦û¿µ;—Ÿˆ4Ü¿á"ÀĀοïÿÂÃ^UNASNone?ïûP•ËòÝ?FòMgŒÖ?B½¨Ð4F?FòMgŒÖ?ïêÖ×.ž?¥€>hÂÓ?e<i(Ñba?¥€>hÂÓ?&^Ë+?†gk¡Ñ`ˆ?ŠZvhM5h?†gk¡Ñ`‡?î"	1BÇ?–Ÿ¾wË?§¿lëӏ?–Ÿ¾wË4FGL J1030.7+6118¿ïù¨.v¶_@HBã¼ÓZ†À:pöa7À;ÐÑPÀô@>/»"zù@™……žÙ?Âc'¦b*¿¦¿$ÝHß²?çgºú<q @ÐË}í@¶?ïðL2Þ¿èò‰?.i¿éüp>–©¿×ÿÞ<`Ù_¿ïÿþªJl¿ß&|¡;N‹UNASNone?ïã¥?®Oî?v¬Q.Zó?lZÀQ°??v¬Q.Zó?ïÕ¥'"¥}?""4Ú<"?u-75­A´?""4Ú<"?î¹£-"lü?›Jp†ŠÝ?¤eÍ&É0N?›Jp†ŠÞ?ï~êiùìì?€QØK®î§?"²ÀÂbo?€QØK®î§4FGL J1032.0+5725?žò2a–@I"~bÜn+À;<Uw*ÙÈÀ<†±	¢@@(²-9I"@ü¦y{ìà?ÐPP~?ª÷J=ªŸ??ÜÞÔa@·«?쥗•C¯¾¿åŸRu¿é|CG}m¿ã à_Ñ¡É¿å18‡0
Š¿ïù
By!T¿ÔcÃHê€UNASNone?ïí»b•º?Ÿn4Œ1Á?bDjúE-?Ÿn4Œ1À?ìõzm†;?ÃCœz±Kµ?¸T,""Î+?ÃCœz±Kµ?ïY<J¿›f?Œeï#¶V?"Øv¨",?Œeï#¶X?êuÙȕ±u?®'*9zt?Æ(˜Ý©:-?®'*9zu4FGL J1036.3-5833e¿ïcˆ®½¿Ç;»cÀ5õÆâ¨eÀ9~ƒujæ(@ ï'v"ò?þAZ=c8?"+¹äŠ%*?¢˜ÕÏTçc@ü†~3â†@H¦³2œà¿é\P˜žÇ×?ڮפJD¿Ü
Æ(Ä¿Úª¨ À€¿ãʍÜÕ¿Ø\$"ô÷ŽUNASNone2FGL J1036.4-5828c?ï¹<[Lâ?µìŠ€fC´?žˆØt–c¬?µìŠ€fC´?ë:²·³:J?Ðø¸JÝ?Ã5!3Ù?Ðø¸JÝ?éÐr¦™?±ÁûIšR?Ⱦ7e›ª?±ÁûIšR?ìu– Äؖ?´Pº«ò)?¼SJùÙ;P?´Pº«ò)4FGL J1036.5-1809?ë6*ürb@AÃ\á'À:Ž%ߍ™±À<^E¾P2G@^û+9À@P1ônÒ?ÂäºiÈƃ?¬Bþ'Q?æMΊ<."@<>5šÁ¿Ó¢<UpË¿å««Ÿ«y¿êJ0'|G¿æÝ´"9¼¿î~"_¦XÅ¿ïìt½—$ÊUNASNone?ïç»i)"?fŸ\*Û`+?håD–ÖkÁ?fŸ\*Û`(?ïäñ…ü\Š?‡ñ€þ?kz£vs?‡ñ€þ?ïµ(ÌÞX?óTÆÖÔ¢?'µÌüÈj-?óTÆÖÔ¡?ï¦-?DD?sÅ›(?†t°.îþ-?sÅ›)4FGL J1036.6-4349¿ä
Hû›n@):ïÔ8ÑÙÀ:Q-ÛÛ]‰À<Ab8Ú<!@­'¦Û÷b@CptÙÇ?À2­Ò5ÂZ?˗ä£-A,@	,辚Úâ?ý=e?tà¿Àõ5v¯_¿Þi%}½ðç¿ÛK-zâtT¿ã?Âùt7¿è¥¶ÞMþ'¿ðUNASNone3FGL J1036.4-4348?ädomp7?ÊuD%?×7!%ݐ?ÊuD%?åK:•ÁÝ?ÐO¬£hI?ÕiŊÔ|F?ÐO¬£hI?äC­BB¨1?ºó.yn0Ý?×x¥{z¯ž?ºó.yn0Þ?æìšÏ¤¼Ú?©lx)Õµê?Ò&Ê`¶†L?©lx)Õµê4FGL J1037.8-5810c¿ïK4::?Ï7äGè¡êÀ8¹Š>²Ã6À:_SUªL@±Ìp±m÷@z…\ '?ÁBL€·'?Òã%Ô¥ß@=B€®?ùÝ(¼Ü¿äÇÍ¿;Ò¿Û*«º®g1¿çƒhÀ2à}¿èeÌþJô¿ï›^?ÑQ¿ï¼~Æ.£UNASNone3FGL J1039.1-58094?•½4!/O?ž²þãƒ?ïR^ö…‡?ž²þãƒ?®ƒwªtìç?¿§ÃÈt#?îȅX±1?¿§ÃÈt"?³¶ŒáHqø?¦"Õ¦kª½?í‰.cÖñÁ?¦"Õ¦kª½?'Ñ=\ØJ¤?qQFòc5¶?ï´»
ŒžÖ?qQFòc5¶4FGL J1039.2+3258?žƒ52,Ca@Nvߤ?åÉÀ:¯û–ä³sÀ<©J–ý'@ҏ7@.@ŽIW?ÀT;ª·#?³Ryt‹K?ð4äù}@³¨Ž?ïÃùߪu	¿ÏZ|ù$ïy¿èL%r€P¿åOàèãƒÈ¿ç|ô¢©¸¡¿ïÿ€H»ÊUNASNone?ïµÍ'euß?'P¥»û?'Œ¶&¢ˆ?'P¥»û?ïÚ®W?ˆg"Îr+?röu¨õԈ?ˆg"Îr+?ï±?ǔ?'= nNKp?)ØÇ
s?'= nNKp?îz®wNy?"Ë
ÖkM?¨UŽm?"Ë
ÖkM4FGL J1043.0+5316?ç!WH¼@K[è>BZîÀ:ØâäfF†À<¶˜x1j@Ā=¨;@ˆœT?ÃO ;Ê0?Žü>:´m?Äàw9@@œ¶"‹ë¿¶ôŒÚC'â¿ãÝDÿŽk¿í2¬'ª¿ÚiVpOu¿íO|	eÚO?ÓH>Þ:KUNASNone?ïæ7-u¡\?zÔv¥U?iÈҊ^£T?zÔv¥U?ïîŸo¤Êr?ƒ.Å&ì£?a`[5Ž[?ƒ.Å&ì¢?ï¿)tÓº?€†í.²é?€ 5¢ËY?€†í.²é?ï몧ÃQË?YåØ%´6X?dUX<®5ä?YåØ%´6X4FGL J1044.5-1439?Ô˜þ^¡C@C©~+VÀ:ãwúã`À<uMËdíÀ@qÃ/?¨@CQÞïå?ϵ»£¯?¿3çmår?ðŽ†@ €?ú¶Qô¿äß,D+©¿æg öo³¿Öe:´e¿é
¸UFƒr¿åà#¡oÑÊ¿ïäê›íUNASNone?ïä欆l4?hu¸f¦ž?kSy"Ë?hu¸f¦›?︼¹Ÿæ?•¯Ù¤ˆ2³?ÐÿQ˜b?•¯Ù¤ˆ2²?ïD1k×UF?|«†:¯´?—y҅WT?|«†:¯µ?î'@mÆÜ5?X¡ôFÏ?¦ëù#'<ª?X¡ôFÏ4FGL J1046.7-6010?༩Ž-#Ž¿îócښë©À8"k·ÞþþÀ:lµ…ˆj@9Œ‹"Y@ÕC/Ш?½Ï€±@TY?Øm©PÆÂ@ܚ )֓@MNB«Ì¿ã:©´™Ð ¿Äo-ŸËaé¿âÍQ¢4è¿ê_Á†"¿íA(¿<¿ïÿÿÊPËUNASNone3FGL J1047.3-6005?†¹~ë ?µgäºÄjÍ?說"T?µgäºÄjÍ?'ú'WÛ^?¦&NJD‡ÿ?ïp+mC%?¦&NJD‡ÿ?'~É1¥Ð}? @
Gj3?ït	¶rÑ|? @
Gj4?tΣeËA?cX'&'?ïÖb¹4iÈ?cX'&'4FGL J1047.2+6740?ä46,jR@F­…ƒb°À;xTFŸÀ=å‡ó@ y¨ä^˜?ü'Dc_–?ÉXOwa‹`?¸.çI$â
?ðêÜ0@	LG²òA¿í$¼B;
ó¿áÁƒ(yF¿Þ€žÐe3¿â@¬ÞDïH?˜·G.%5¿êq=Å]lÃUNASNone?ïÿ'–›ÚÙ?{6؞G?šY	I;?{6؞Ž?ïþc%ÌL?Gè{ æ‹?/éÍ£;?h?Gè{ æ‹)?ïðÒ¡ñ?q¸7<M>?_ïÆZ¼Ñ?q¸7<MA?ïþýl½ ?£nÞ=ê? )3Ô%÷h?£nÞ=ù4FGL J1048.4-5030?àe¢ï:±'@èϦ›áÀ;~‡Å[¿À<€"Œê^®@"ží'`A3?÷&Lëk…?Ùޘ§+R"?Ò¹Ù« ê@•‰ïØj@@7Ӏñ¿Ó@LyË¿ài}Èâ¿ä§ü~Y®¿äHxÌE¿èè\૦â¿éMŠ'$‡õUNASNone?ï¡7€BO?†¾Õ,oˆ?‡²ïl: ?†¾Õ,o‡?îvy ²Ç?§£Ë…®?®¨˜môӐ?§£Ë…®?îd4Ê°?žK"+ZL?®y¼³_Äó?žK"+ZM?ìm"ðõFS?°¸œK<b_?¼"ØxUÍh?°¸œK<b_4FGL J1048.5-5923?ØÚç¡X‡ñ¿ÅU€e-À8µýawÀ:Œd×-©@Ì22Yò@9fâ?¿äð/'ŠÞ?à€`b–M4@èîkƒÙ?øœ¤Z诿ݫ^ʐ²¿áa%Ie¤ ¿×ÐfíÖÞ¿êS恩¸Ì¿ïÿÞý¦ßR?ïùT_}¾óUNASNone?y
|'t¬?Œ9ÜÓµ_]?ïÍåj‡?Œ9ÜÓµ_^?–y愔\½?²‡šRv¸?ïL0ËÛ]?²‡šRv¸?£Ìð9¡À7?š¤‡I?îÃ0üeãý?š¤‡K?4qôd_ÁH?,d°¶Ü¨?ïýqÁst?,d°¶Ü¨4FGL J1049.8+2741¿ì݈ÀÏo@O‰\Rç-¡À;$jÈ˶LÀ<ÂÉø6{@Èey+ü@c'†Wv?Á?wd:'"¿ª†»›w_?ê_
Awn¡@Qu=™¿?ï¤nß±¬¿é£=òÔÉ¿át€Û\²ˆ¿ÞCO
)N®¿èê¢5Ié?i…ÖüíUNASNone?ïíAR}ƒ?[ÌD¬´˜?bp¾­'}C?[ÌD¬´š?ïûÅ¡TY˜?c–öb§I?@éz®™£?c–öb§I?ïË]âaR?~m†j…=ð?zQÏVý>?~m†j…=ô?ïغ‹ØÙ?`·˜‰%ï?sø"º"?`·˜‰%ð4FGL J1049.9-3658?àù×4@3ÒóÂÚۃÀ;o…j7¬?À<½¯€‹¬@ü<'UÓ?þ#Ÿý`éO?×îS/Qý?Õ<캨ÝÚ?þs™õßëŽ@nÏ[rl"¿Îˆ""ꐭ¿ì6J	8æ?áO܁u¶f¿âÉ­"K¡¿¿Úû¯cZm_¿ïý_ ÷ÇLUNASNone?ïèô¢àØË?høÀÑGf?g]'5?høÀÑGf?ïúˆµ÷.?g?¸4–?GáÝ(#G ?g?¸4'?ïId4t1ð?ÿLù³‹å?–ÓyqyÁü?ÿLù³‹ç?チ¨Uá…?nAì0]æé?€_•ê‡ž™?nAì0]ææ4FGL J1054.0-5938?ìøFŸq9ª¿´ê}6âjÀ:*&¨«À;zKìgœÇ@¥ðj
à¯@DÍ$
¡D?Ò=Äòø6?ÛFuš¶Ð@	Ž"ü¡¦®?ÿ[Fo¦/¿â¿°"—ª¿ààŠï²ªã¿ã ¢Bµ‡¿àýT‰Å@¿ì¯¹"<¿ðUNASNone?áÑPךs?Ê(9e~,>?Ýô]^PË?Ê(9e~,=?ٍ•ãý?°?ÕBY9?ã95`(?ÕBY9?Ö%}Ì×¾?¶½MURJæ?äõmA"!?¶½MURJæ?ܪº7$N¶?¹%<éëC?᪢ämØ¥?¹%<éëD4FGL J1054.7-6008c?ï«D ¿ßt_ƒVRÀ9>¡ò-¯fÀ:ºôƒÊû;@ ¬ÿ"Ë(³@#éÁЈ?Åß¼™Ï?´}áWHfK?ôc@\¢@x•±'™¿é–:‰hÊ?î6êx´G¿ëB‹`òË¿á…!ýÖ¯û¿äw'¯c¿éÎf*…UNASNone3FGL J1054.7-60064?ë]†¥û¯©?àގ¼"Ì?‰åhA^?àގ¼"Ì?äcÎwsc?֋¹Ùð?×ç8c8?֋¹Ùð?çáDp	`H?¾³…j€3X?Ð=wí?q?¾³…j€3X?êtëX‰}?µ]éd?Æ,RÛ†	?µ]éd4FGL J1055.6-0719¿Ú'IÚYIÞ@FË  ôØÀ:Òs«ÉGÀ<}4#;z@öõtŒ?úfÉèì¾?呈pSO?ãè›)¼'ì?ýR0",J@"B)›.ð?ï¸;Ÿé?¿á jÓ¿Þ*¤ ¿í·¬ª–¿ïêԟ©þí¿ïýÁÆßMUNASNone?ï±&,¬s?Él£ÐO?ƒ¶túÔãh?Él£ÐO?ïˆQàîmV?§^Bi¶?ë‡Ädªt?§^Bi¶?ìt¬¾š'ò?£ß¸Óè«?¼Zš+pu?£ß¸Óèª?ìÙ­í#â'?¨ñ"³Ål\?¹2–àîÇ?¨ñ"³Ål\4FGL J1055.7+1033?ïߘýjψ@M¶0©8À;mv"Û·À<·þ^?Px@L)ÿ'׋@Õ`EK?Îú0³&2š?Šæ
²ûj?¸åõåZ¸@xއ_ZY?ë;>À<{¿ê©p§2'?²zò9˜Ó¿áöRš™Ê¿àsø^K¿ï—m¿öûuUNASNone?ïþ¶¾F¥%?"w-·7UÄ?$"•­¹°?"w-·7U°?ïý­á?<?L77²bû<?2öod?L77²bû"?ïíCKúdf?qÂ@¿4'Y?b¼´›˜ç?qÂ@¿4']?ïù$Æiˆ?9?ó¢Qñö?KÃlæYÞÒ?9?ó¢Qñü4FGL J1055.7-1807¿äs*fr@Bb¢"ÕÀ;†PÎN­À<¦üZYê@`àëgÃ@T"\Böö?Å
{"Üß¿·Y ¾Í–Ý?óUE¬²{@'óÒö­?ï'S‰êÏí¿ìîbHŸ¿áé€C‡>¿ã")Zl] ¿ÏfD˜
xT¿Í^;I­UNASNone?ïèa;di˜?_ßBí*Õ?gžÄ›–hÁ?_ßBí*ß?ïü%?×??[~ŽÀðŸP?>ÖG%û	?[~ŽÀðŸT?ïÃ>¿Eܬ?'§~/~·'?~` ]©©?'§~/~·?ïái°Ýci?aV}"ý6Ÿ?n–O"œ–Z?aV}"ý6›4FGL J1057.6-4051¿×£,á@1«\9¼ºÀ;T'ÏR¹
À<¯ík¨Å‡@!Å.	¹?÷ÏY­€?ÕÛt/|ÅM?×­ãænß@®¤Ã™Gd@ЈÐº%¿ïÿóÀ¬ƒ?ïÿÿ&¦³?Üe·>ñŠ?œÖƒb~-
¿Þqá">éu¿ãJ½Y<\UNASNone3FGL J1057.6-4051?ïýú̀äž?+bþ\álm?0)"øÛŽ?+bþ\ál_?ï÷`Œoàî?wp^c·Ûú?Q>ç >&ç?wp^c·Ûû?リõË@š?	¤[xR?€Y/َ?	¤[xR?ïÕ¨úß»Ö?d5‡×'ý?u+'"M?d5‡×'ÿ4FGL J1058.4-6625¿ïQØMáõ$Àú†×6&À:©ˆúååÀ<@—ŸÄV@ –|¨È?þÄâ½ÏÙÈ?Â%;8eL5?µ¦?piu?öóFc'ŸÐ@à¦ÉWø:¿ä|Wisa?ïò±}»í¿æŒ"ÎX¾¿Ò¤e¥vF®¿æ,SzÑWv¿ÙÞ¾‰¾UNASNone2FGL J1058.7-6621?ïòÿÇéëœ?TǦ?,lè?Zp,(È?TǦ?,lÜ?ïÞÖÁhÌ/?"ôlèF¾ç?p"ŸK™çÙ?"ôlèF¾è?酪Z¬ÿd?‡ïm2¤b?†Ù©TÀ&ø?‡ïm2¤b?îٰۀI‰?'yÜ`MV?¢dòGûgg?'yÜ`MU4FGL J1058.9-6101?èZh"h¿ñ"ӟNå@À9¢G«<#À;$•%–'~@…¿9fS@÷xmži?Êðmü1ê3?ԘL½rç©@™È î!±?÷ê–߀Å¿ïÿ¸8º1?ïøVˆ¢ÑQ¿à2Û>Õ}Ë¿ã<æp–¿ï—_'œ}?жƒ_E‹UNASNone3FGL J1058.5-6106c?Æ,®''?D?Âç½
³áÇ?êtÔ[_p/?Âç½
³áÇ?ÈÆýÝì®?ÎðΓױ?éÎ@ˆºDÔ?ÎðΓױ?λàeDð?´¶<Qrë?èQæ®Ãú?´¶<Qrë?´tùÖUL?¤Ü 4§ªÀ?íq`Å5_?¤Ü 4§ªÁ4FGL J1059.4+2148?Í!ñ:jk@P,{‰
ZÀ;N1‰åÇpÀ<•ÀY÷Ã@ddàÕBg@îà¹Ü?З¶€G7?¹d
ý´÷?èñ'?_‡?ìKV^~ª¿Òn¡¾/•¿ã­`öºÝ¿âл¿^OA¿éšº–icq¿Ê÷‡‹z¿ïñd "‰UNASNone?ïéĘ6§?Ÿèº8HØ)?f;úgÉY?Ÿèº8HØ)?î°FÝrz?²ƒ€ZQ¡O?¤û'(Ø_Ä?²ƒ€ZQ¡P?ïr¥'ü?Ž!^tAÞ½?'«_¯ y?Ž!^tAÞÀ?ì_ìEXѪ?«s#‰?½Õ9r¸?«s#‰4FGL J1059.4+0226?ë]R	n‹u@JɏÙý7À9ÞkÑà2À;òhÒQq@‡séèw@½‡Ý¯s ?ÄåýJn
O?Á9ul"§?öÿ\‰ÉB@I¡yŒÞË?ïÎ` ©®¿ßè©¢%YV¿ßÙ=ˆ÷Šæ¿ãX{Â=ä¿ë²‰ŠWÝ7¿ÞAÜCbU`UNASNone3FGL J1059.3+0224?ïk׶vŸþ?¡ã"šãp%?'…	1,)?¡ã"šãp%?ï÷aúqRó?dĀ›uH?Q<Z%?dĀ›uJ?îˆ;²Ký?š»6
îH}?§|Dß{@0?š»6
îH|?ï4¼ÊÛ?';:ôð?™~(f¤?';:ôð4FGL J1100.0-2044?ëù£æÛs@A‡´€¥¬ÍÀ:ÁçIOÕ*À<"÷z€Ï@@¸žÂx`@SÕ4z[?ÆÆl ¾4?¼C"Ó†û1?ñu~æ­?÷µ×8XŒ¿Õé4 G3¿ãgšx
ÿ¿Ùsÿ*¿åÑG@~š¿ãæàtI~¿é¼«aÃ'UNASNone3FGL J1100.2-2044?ïçWû(•Å?cVøx(•?h¨×j;R?cVøx(?ï˜*'ôT?›Z'ù¸Õ‡?‰þõ[Bë?›Z'ù¸Õ†?ï¦<x'O¤?"H^EM
ê?†páö,?"H^EM
é?íìÚ7cˆ‰?•ˆŸ¹œQ¼?°™.Dã»»?•ˆŸ¹œQ¼4FGL J1102.3+6715?íÙ/<N5®@GJ²BÀ;è¤nòÀ=0fC*÷û@!PØ?ɵ?ûV³»ƒÏ-?ÏAÖçØÂ?¶î•ÊW&­?êö5çB™Ù@ÓLÙ!™Ù¿ï¥íÀ7h!¿Ô°oó ?ïù0¾
í)¿æ{›¢|K?¸Ï2ؚ`¿é8%@+i:UNASNone?ïÿcJÏߦ? /¼2=•?–¦CÑ? /¼2=•?ïýþ!̞?H¬Yî™?0ô›X?H¬Yî˜?ïÄÄeän?ƒ.Û!T!?}óÍ
É/?ƒ.Û!T!?ïþºO²? ñ17{²e?'ï[ÚB? ñ17{²L4FGL J1105.1-2600?®éœ·1÷@?â2ŸÀ:ŸÀgnÀ<'•=†Æ@'ñ§Lµ@(í½\ì?Пª?ÂpŽHÌ^?óå3E§©þ@ÛÃ_»§a¿àÕd¶býü¿æ6ü¡%Ôü¿Û"ɾO†{¿ã/ýÍpa¿ïÿoì÷å¿ë¡;NŠ§ŽUNASNone?ïâwá2ð ?m¾ÝŸì"¤?mˆÍ`1?m¾ÝŸì"¨?ïû-‡Å:u?^Í׋»Šc?CIàë,?^Í׋»Ši?ï$¼8:§Ö?"ñÑXÐ?›hxø«9?"ñÑXÐ?ï¦i"›<¬?qô½âP?†e·Y0Õ?qô½âP4FGL J1105.3-0626¿ã¾7š#w*@Gß÷øʂÀ;¢HÕ[èÀ<´Ãð…8º@#P׿ïï'?³k=¯:@?çµ+ÆWh?ïÿKÚÉå'@""†âÞ?þ¾+õ&]¿ïúìšÈmÂ?ïØQ?¸§§¿ØŸ½J"ä¿êèD§¯Ý?æÑò¦{)l¿Í¶¥CÃUNASNone?ïUicºùg?¤ª½^ƒ?•Rӈ Ó?¤ª½^ƒ?ïólŵ¼.?ƒÆXB¶ìÅ?Y&t"‡¤þ?ƒÆXB¶ìÅ?íDñ¬õM?¢ÌޓÄPÀ?µØwژUš?¢ÌޓÄPÁ?ïÒ×6®?€üOÀÈ/À?vÿd¨öî?€üOÀÈ/Á4FGL J1106.2+7303?ሁŠ·œ@DüM:'£À;þ#qõÀ<5‹¶'@'Ÿ‹¡y@ãÏ¥Å!?Å^BÀïÉÒ¿»'¹5Á-?õÀ´á¼©@«'â[?×}_*ÝÏ¿ë3™àf\«¿í~ÞAê05¿—'n¯¿é[Ŏ*Y¿ïæöäÎKRUNASNone?ïÚ´µ‰ƒ°?v[:GžT]?r¥¥;>(R?v[:GžT]?ïv¸EÙiÇ?¨·¢s·y?'(÷DÒÇ?¨·¢s·x?ïpÞÎY^€?Š):Iý|?'ä&4Ô0?Š):Iý|?ï¯àÂ#ò?}̏€i?":GÏwq?}̏€h4FGL J1106.7+3623?·mTþ¯	@PŠ\å´$À:|ƃÝo²À<]˽Ù@ø³"כ]@îwÐÛ?Áq56î~£?¡Œ ?ƒ¬%?ÞwÒ>Nš@m«ÿøž?ïÿÎa¢\a¿àÏÜKÅÑ0¿æ÷ôގÁ#¿âÝ­Å ˆ¡¿èך@]".¿ïþ!nÑTUNASNone?ïþNúœåg?$÷æ]£?+V1©‹Û?$÷æ]£R?ïýXŸâøm?O'xB0BS?5;è<¤Q?O'xB0BG?ïØùñf?tÕ)ñ7|Ä?sƒ9LÿŠ?tÕ)ñ7|É?ïý ‹&Ð?"àÚÎ9Â
?2û¦Éì?"àÚÎ9Áë4FGL J1106.7-1742?îv;N÷·Í@C=À~à±À:xø‹—xWÀ<†]Ötì@‰ú‡;?þë'*ç?Ãì[!Ý?Ùh$¬‡³@pÀ\|@Í¥u«¿æ¤;~[O²¿¥~ŸBP©¿Ö¼ð¡=Qð¿äó;Ì_¿ìƒlfZ§ì¿ðUNASNone3FGL J1106.6-1744?џ‰âŒ'Ñ?È;ïqLãá?ç0;¹ì?È;ïqLãá?çIèJXÖ>?ÒËpžÒÃ??Ñl/kNSƒ?ÒËpžÒÃ>?±µÃak§Æ?¢µ¦*ü?íÉG"Ò‹?¢µ¦*ü?åï`f€©¤?³]pƒ/%?Ô!?2þ¬·?³]pƒ/%4FGL J1109.1-4853¿îëãÚnŽE@%8ñ,'¦7À:eÒ(V`_À<,"d®ÖB@ˆ¿¬¨À@Ùýñ7?Ϥ4<ȈE?àãm"BJ@€˜@Ô¦@lLJ±T ¿Ê˜ÊÔпÀ'/Cå]¿âz•ÈSÁ¿â*þ~ð¿ïڋÒ0¹Ü?욉¹QÅÅUNASNone?ÝÐÚÄvëÏ?É×zï&#C?á'ÄŠ?É×zï&#C?é°Û>1á´?Ώ³qAé?É<"8y/?Ώ³qAè?ãmG(h]þ?¶÷&Èߢ?Ù%q¯/D?¶÷&Èߣ?êvÔςi?°uìï9G?Æ$¬Áö[ä?°uìï9G4FGL J1109.4-6115e¿Ø,"zеs¿èÑØ8såÀ7C9+À9ãKÁŸr@!ÿr:Uf?þÝí¡Xª¼?£&"S¼ì?¦¯
šÜ@@Sý®(?òIK :?îT­×>?׿à'°+¬V5¿ßc? (ÿԿۛ㪵¿ãÍ®oê¿ÚpMû‹| UNASNone3FGL J1111.9-6038?àGƨèž*?ÏςQ;.?ßpr®.ì?ÏςQ;.?¸'ŠoÚœ?ËÎYñ2KÚ?ìíβ½m?ËÎYñ2KÚ?ätÊö3êª?¸õhìuÊÆ?×j˜*¬?¸õhìuÊÆ?'k±ÜQ	?Šõo½#?ïl§Rqx?Šõo½#4FGL J1109.8+4406¿ïÿ©hì@O»\6À:À@æzýÀ<±*_Oð@WŸ
ÌÇC@ñ¦Ö˜þi?Äá~_¬bõ?°¥¸¶ÀF?ä»[áF×?ù¹99²~B?ì‡À=È7'¿ç"y߿éÅEŸFÅ¿î!çEôÖ׿ïÿµ¿Ö̯›Ž'SUNASNone?ï÷s:"?[Y@šQÊ~?Q狼}?[Y@šQʂ?ìð·³ñ?Ã1ŒeªÂ?¸zGzgÐ?Ã1ŒeªÂ?ïI®!K+j?a§ä1dC?–Ê;֚'Å?a§ä1dD?꫓4eà!?µÔS±§Ál?ÅQ³.h}?µÔS±§Ál4FGL J1110.4-8023¿ïxz'l¯UÀ2aA…ÞÀ;k‰lû«ÝÀ<°±¤RZ@@!ŽUºF¸K?ó¹Ef;ž<?ÛÀÚ»¢ØÝ?éöh§‰Fe@"å$²fð@2¾/%1"¿ïÎ8<‡oË¿ísXHÕ\¿åš\!¾ì?ïgõbLM¿Ô1©ñb¿ïÿæŸÜ©ºUNASNone?ïégÚJ-?i÷Îàý
Ð?f˜%µÒp
?i÷Îàý
Ì?ïí½B§:ƒ?"n!}€ª?bB½XÅ|_?"n!}€ª?ï'Å?"À±¨)Ì?Ÿ~½‡]˜?"À±¨)Í?ïÔQ®÷ª–?xO«­?u×("*µ#?xO«­4FGL J1111.4+0137¿á<SyÎÐ@K€`VìÕÀ;'‹®ŒÀ<bjáö)½@û}9f©@XdàTi?ÊÍG›õêR¿=ugÓQ_ê?˜ã#¶V5?ùðrƒÖ
é?ïîtÝw"â¿ëqBb{[¿è&Ï!»¼"¿ÔÈUÚ'(c¿ç–Háñ!@¿ïù&A³(·UNASNone?ïù"ÇÌî=?Gkc#*v?I¬àÌG	ã?Gkc#*}?ïÆæ÷¥#¦?"™¯QÇ/R?|Œ"-n,Ë?"™¯QÇ/S?ï¨ñ
¾¦…?Š¦ÙrO?…üV^ž?Š¦ÙrM?ï6ÒõÀùw?†–ÅXÞ?™%¡GàÑ(?†–ÅXÞ4FGL J1112.0+1021?Ô#?€{ÑT@N›‰
Z[–À:²˜ˆøa¦À<beÀN9I@ž¡@W@	z¾A?ÈlxÏ¿®•ûÝå©?×¥_ yˆ?ÿã&«esø¿ÝÏI~Ïø¿éu¢¿<_¿ïaß¹8›R¿ë"ãw3=D?ì.rýMž¿ïÿÒ³–šâUNASNone3FGL J1112.1+1034?ïóðšøM?eàÿ-ƒ?XÊûe¯?eàÿ-?ïó?a_y?ŒÕªül?Yρ=AÃ?ŒÕªül?ï8Oß®°?'i\¤žþØ?˜öä
)ñ?'i\¤žþÚ?ïúÆl)kf?GõÊå99ó?DæOZRfì?GõÊå99õ4FGL J1112.2-6055¿áVqBñ¿Õ8;SéÀ8¤à·e\{À:)1™Õÿ{@ 
y#ŒÈ@­'hr°!?ʚ_,
u?ÓOW xEŒ@T>S!æ?úyLò÷ÙÁ¿îg8¿d?¿ãÎ_ã¯+¿Ôv§ý	«z¿æ¿£ƒþ&â¿éR½g)/¿ï+4+€·KUNASNone3FGL J1111.9-6058?"sÖð†}?¢­8盧š?ï®0¤?¹å?¢­8盧›?'(º6·¢Û?¤¾­ˆo??ïnº.JBé?¤¾­ˆo??´Z$:¯3?¢¬lؙ>?ít»xª
ú?¢¬lؙ=?p˜ HbA˜?d-¹>Æ.?ïÞοo;}?d-¹>Æ.4FGL J1114.6+1225¿çi¢Ñ#s&@O}Ëݹ"À;dÑ~uYÀ<›ç+ä<@g}ÕÃÁ`?ôFâ!ȧ¤?àþ'î?ïÿqÐ&ô@Ø®$kT@I§¾ËW?ï<m¿ ;à¿î»+à-§®?Òa¼­ž¿Ö‡KMÜ+å¿ïÿójÆGx?ä"e}2ZÆUNASNone?ï´²/sé?†(¥BÁ`C?'úSt#¸?†(¥BÁ`C?ï¤ñÔ¿Ö²?¥eù:Fw?†ÃŠÐ
Sš?¥eù:Fv?í¶(«²f? óSQvô«?²O^º¢lÇ? óSQvô¬?í–MµÝÝ?¨@ŸPIs?³M'Qñ?¨@ŸPIs4FGL J1115.1-6118¿ëˆñ…BK¿â-tw¡!MÀ8D~ïÊ'×À:
ž¿s@ rHqß@Öº;А§?³¾R`Ÿýâ?ª‹~g¨Ê?ùãòhgÈf@"³U?ìŠ@Ë¢*b¿ãÆ
`:Ó;¿ẩæž/+¿ç'¼£n¿ä˜êýºU|¿à5몥çUNASNone1FGL J1115.2-6124c?áîV_ð?Ð@ç
I{?Ü#S@ ?Ð@ç
I{?än°F a…?Րs4w)?×"Ÿr¿<õ?Րs4w)?âú=dÁùj?…DL¬'¥?Ú…6|
-?…DL¬'¥?Ý¢þ+Zœ?¼á:á¤?ás®€êR²?¼á:á¤4FGL J1119.9-1007?Ü:twƚ@GQµc#»ÇÀ:ë浬×À<b¢Œ‡b@N-ۅw?ÿX×1ª?Ñ+û›í0ð?΁ûWϟ»?üöË #÷@	^0;;X?¼äaئä¿ëY:>b¹¿Ã;Û"zÿ%¿á¦ßîÁ¿èRàýÜ9Q¿ïÛ`í*»UNASNone?ïú]šÊ[?EW,¬È?F‰"×ò'µ?EW,¬È?ïý&!¦?NÁ"ôUã?6ÌñêÏ1?NÁ"ôUä?ï˜u"à;Ý?†µ•f÷F?‰â›ñ¨?†µ•f÷E?ïâUdV¢?Sž½Dª?mª›o©]o?Sž½D®4FGL J1120.0-2204?ïûÅØ¥")@B(ÂzÀ8Ígi›¥
À<ø¨ê@Þ}˜19´?üæ+ÈÛ¦"?«µÊ|»gu?Þäµ—&"@/êjP
@•'æxðW?ïùÙ?¡Ö¿¶UŒ_°zî¿Ý£¦ï¿è"kdÒè¿ïÿûbâMh¿ïæó{?UNASNone3FGL J1119.9-2204?Ä\¡ûï'?Ð4ûá8?êè×½Á?Ð4ûá8?€"e_'Ë?‡Åisö\?ï¿vj·ä?‡Åisö]?·H­)È6N?¥½ìÐ(âŒ?íêZÆù5?¥½ìÐ(âŒ>Ð))¡•ŽV>ÓQ5'D?ïÿ÷ëk/5>ÓQ5'D4FGL J1120.1-2645¿è}w|@?Ï>$þ½
À:GXS~,VÀ<_'fÅ0÷@÷´Lù,ý?þèõÝgNÄ?º/÷¿i·Õ?ƒlßHǼd?ÊaÁ'ýö@­¨ñ{Wå¿Ù‹Q¢Š$¿ã5æzyC¿Ü팈†w¿ßœ7£Û;û¿â6þ™Îs¿«P'	ÚoUNASNone3FGL J1119.8-2647?ïþ¥%Wµ?à@îÅTò?%®Mª"¡ï?à@îÅTx?ïþY'ì?D2ä¸Â¹8?*g×î?þ?D2ä¸Â¹*?ïú¯íaB?Z8þËç<?E@Jz÷Ê??Z8þËçB?ïúÚÞ4XL?3Q)8õ]?D"‡.žÍí?3Q)8õj4FGL J1122.0-0231?ì.·+ÎGZ@J¬wFˆzÀ:õQ³PúÄÀ<Cb?8È@Šx•½ìà@c줩(?½É¹ÇâWN¿»é\`º;6@k:á}]ú@ܨX¤0÷¿å•b'¬K¿å6fœí¿èð«Ï&C¿åé'yâ¿äû9âyÝ<?Ö¶›Ø'UNASNone?ïß¿m?r뢜SÅ?ps I7ó[?r뢜SÅ?ï#Ä_v¹X?´#vnšå?›‡t(Ôè?´#vnšå?îøE^ÆË?–^¾Õ­þ? {¯:"`?–^¾Õ­ý?ïVG
ƒ%0?‡¦
}G…?•7¯›Yó?‡¦
}G…4FGL J1122.2+3926¿äçaâ·¤ø@PðváÞ¬ÉÀ;(à#Á¦(À<'i<Ú{â@#³—œ"@[iQ;?Çúj"2°¿¡C!£ú׳?ÖQå&µÌ?ü¾#çÈe?Ö_#Æ®¦¿é¢²G‰
¿çXl"h	Õ¿åþ‰¾]¿éPKý"z¤¿ÓUG¥[ÕUNASNone?ïÌFéx<?wnÊHƒ?yõ܋Cáƒ?wnÊHƒ?ïÇóû»j?"‹ ';_Û?|u"Jä?"‹ ';_Û?ïjä£C¢?‰!«Þó?'£k—‹¢?‰!«Þó?ïu•iè`˜?oÖ·O¹÷?'MRÂóí?oÖ·O¹ö4FGL J1122.4-6237¿ç¹]¡‹ì¿ø"ÊL¿ÌÀ9SdžJÀ;
¸ÜU
@ 7~ä6¡@Z¨!ò™?¾ònGx? ÜñC_âO?æ)Ïqºû@I4ý7Σ?î²:zOQw?ïàß¤jٿ媚rÝm.¿èÇ)Š=D¿ÍÀ‡Y¦¿ë	c@—ëUNASNone?î"$€'?ª†nã'JÍ?¦¿­·ýˆ?ª†nã'JÍ?ï¤
P,d‹?¬(0»ò	?†ýkôæÝ??¬(0»ò	?ìµ-ŸI?¯f½(¸èé?ºV"·/?¯f½(¸èé?îXäéKž?ž½ôn¯í?ª~!±kF(?ž½ôn¯í4FGL J1122.5-1440¿íÁМãö@Ezã`'À:‡ànj@æÀ<N&äpX@Þ2>k @|ÿŸ‡ð?Â|ãUzZå?°Bü>l?çu	Ar;1@ꖧ 볿ãOµqfu¿âøÈÔÈ(¿é=ß>ir4¿ìåþÌú6¿ÄçxŸ£ô¼¿Öԓj«o…UNASNone?ïށêDgž?t*§kâè?p¿
ÝÌ1)?t*§kâç?ïøGÒ0­µ?p*Ë,,)(?Nà·=I+)?p*Ë,,)*?ï[°s™E?!w•Ò§í?"‰ñŒ×_V?!w•Ò§ì?ïÑڞã.™?m²dµ´6a?w°Žh³ ?m²dµ´6f4FGL J1123.2-5111?ïרwš±@"š{9&À:¸ÕŸeæÀ<RÂ&@»¡iÍf@NeÙx¬º?θ©?Ñ&?×8´|sîå@·±ÚØÿ
?ü|h±D[¿ïuH¡¯g·?ïé$ò'Ð)¿àL"b¥¼"¿à2kݞ¬(¿é4èªxäî¿ïÿŒ	ß}UNASNone?î{I|µs£?¨x9ÿ¬Õç?¨Kh4¨ÅÙ?¨x9ÿ¬Õç?ä½Ú¯_þ?҃íûðuÈ?քJz¡@?҃íûðuÈ?é€?ûIêU?°ë÷F?ÉÿØVª?°ë÷E?ãÌýNyŽ?·¡R:?Øf÷cã?·¡R:4FGL J1123.8-4552¿²¶1¹P9@,­kD¸ÃÀ:2ϾÕÀ<Hóµnâ6@Œ¾A™¨]@ÜOÜ·%œ?»Ýظ¾M?±g?Õ-'?õ/$*³Ê@qI^BÖi?ïùJYPԿʓÂjU%¿è-YŸ®†'¿à×ewS´¿áÙ[ñ˜^0¿ì"Áœm	UNASNone3FGL J1123.6-4558?ïæõfÁ,?g°ã&ã?i
™~>Ô?g°ã&ã?ïóû(þ?pw°l¶?X	¯ÞúÖ?pw°l¸?ïÎq='6Y?zf´ÇÉä?xÇa>äÓ-?zf´ÇÉä?µ´N*?r$y`6«?R'ìuw?r$y`6©4FGL J1124.1-1203?ŠNøˆùç@FºY!…ÆÀ;+Ÿ'xÀ<•®Ðbƒƒ@Vï|úýb?ÿ!ƒ†Ý?Ü­$ÜtÏ?ä¶öq@"恩¸Ì@ïZÎy¿ïü!~|?ïÜ^o÷ß ¿Ù€¬ã£S¿éCa(¹Þ¿î-‰Û¶tœ¿î¤Q]똕UNASNone?ïwW§èªÅ?"¥Öݲòû?'ê§P?"¥Öݲòú?ï°[CɛŒ?›ñåw/p>?ƒé/
™ñ?›ñåw/p>?ì›~£þ%¢?¤Ò+¿[nl?»$
àÒò?¤Ò+¿[nl?꽉*7?«©šÝ|iˆ?Å	ەûW!?«©šÝ|iˆ4FGL J1125.2+2557¿à…˜›B¿@Q­LD|0ÓÀ:+·=ïOÀ<€¼ÈrÊù@Ùÿ°yÛ@ð@|ÇÑ»?ÄàðZÆu?ÕÁ~gô@	¶§[ùûÚ@rZûÏ×?ïýË<©Ôz¿æ	g½~{0¿é–¹èîl¿ê""½¿ïý²GæHŸ¿ÓО¥2UNASNone?ïðúxß?ˆ]aæ1P?~''ÃñD?ˆ]aæ1P?ìô†
;ÆÍ?Ç*d—à")?¸[Ï®!ɝ?Ç*d—à")?ìÿÕñ¼&R?¤ë!…_1t?¸PrÍt?¤ë!…_1t?éá8?³Ò˜
xqå?˛ø{ÿ£?³Ò˜
xqå4FGL J1126.0-5007?–êA@$ìܨââ¹À;E²à'|oÀ=–"TÛú@˜Õ1 6?ÿoB]r¡Þ?Ó|
}é?ïG}½›¢@ÇVO—î?ý)ºËÃ?ïû²}ì¿æ5‰2C¿È'MÅ°£Ì¿ÒՖŸê³¿ïþÂ^§U¿æU/þËMUNASNone3FGL J1126.8-5001?åzàGÀܤ?Î	3gˆ¾?Õ
?p~F¸?Î	3gˆ¾?­‡å.Ž¥Å?ÂP¿2{s?î'­¤?ÂP¿2{s?Ô];hµHá?¸öʙK?åÑbK¥[?¸öʙK?—+Ääº?†ófsÔ?ïGŽ¡ßxÚ?†ófsÔ4FGL J1127.9-6158¿Û;_½¯Õ5¿åÁ¹óêHÀ8ÿÁõuüÀ:²ÿ%¿­@Òg°"[<@–øAŝ.?ÁÇHhújj?֚ɚh@ߧÃ(]?þk§ùÈ.?ãů¢›¿Û–­@•ql¿ã×ómJ†¿éå9àÌ^¿ì¼í[¸{¿ïòÌ&°nUNASNone?q­J"ZÝ? .z«¢?ïÜ¥jÙýJ? .z«¢?¬ÒK&vJ?½þ5@*ín?î2ÛMŸèœ?½þ5@*ín?"u¸¹>—?‡T¼QIâÈ?ïdR:6D?‡T¼QIâÊ?ƒ-\vs¥D?j©³43?ï³JŽ&1j?j©³43'4FGL J1129.1-5230?ÂüÖ"í¯W@ ´Ž:!dÀ:ËêpKÂvÀ<BW¿¶n@/§J\D¤@#Êŋì?ÁÊZÒbä¿¢E›ÚUe?áKÌQ|ÊV@
ájCÒ ?é|=}¹ê¿ÃJ&¿²]
¿ê……t¿Ù-Aª‹¿ßEqcÅwC¿ãñ" Ü.UNASNone?ïô­Dœoº?WµÂAG¿w?V¥vÇ ‹‰?WµÂAG¿t?ïýà	w?Y¸Ú'ïÐþ?7ÈÿG´OT?Y¸Ú'ïÑ?ïÜÁš."?w"ÓDûL?qó2è¾?w"ÓDûL?ïü"‹Ë?)ÍíÆR×D?;ó_û¡¬P?)ÍíÆR׉4FGL J1130.5+1400?ÏŒBgÀ"@PÁå!WhÀ:È£öꭈÀ<r5r
	@a
þw¥@îùûA?Äm¦ß'm?jF/Ä{µý? ÕÇóE:@ýClç4¿å¾¬#¿æƒŠT'¿åGxÏõv9¿è|üÀZxœ¿éÒŠÝ>4¿ïmè jUNASNone?ïüu›Åÿê?8²1s¹z?<S!ЬH?8²1s¹`?ïý:AvOÓ?P=·Y'â?6-ôM`y?P=·Y'Ù?ïäòMälÖ?n.•!Ó¨?k
²"*Š?n.•!Ó¥?ïõÕܵ‹Ç?D,2Ä ì?TTF"ès·?D,2Ä ì"4FGL J1132.1-1448?ëM߯œ@EgÀ:÷nªØ†>À<ræY¶U@ #3ºÂ‰'@¸ù±1f?ÐB¬©—?¼¶ðÂuZö?ñ åRՏê@3¹ˆw]Z?¤àA@{?ÒD4¢Éî÷¿å.â q¶¿Ñ²;{+¿ßö'þ¢ˆ¿ïþù:!EUNASNone?ïþ€Gû›¡?'.‡x&›?'û€FEç?'.‡x&Ç?ïýº¸Á?R_¼÷iÏB?7Ò/š:/?R_¼÷iÏB?ïïnÚÊé?eÛK{Íä?`'%å5r?eÛK{Íã?ïç$&U–Ã?TؘЊqý?hÛÙªi=}?TؘЊqþ4FGL J1138.4-3555¿å(ìD$@8¥à?pXÀ:Ì<Ý ·À<{(7V®b@ؽ›×a@Bý@27?ÐâÛ¬äz?Ó(.rýN@ä%C†gŽ@`'ÿ÷q'¿åív% Jù?ïý»ýœ£d¿âRÞt?¿âw8¡Jr¿ïú?–më¿ïÔ. §TîUNASNone?ï؀n!Æ×?wáí˜òm?s¿Èï"´?wáí˜òl?ïڎRØ׍?˜°~)O·Ú?r¸Ö""9q?˜°~)O·Ú?í}»ô-½ã?¡Ì_fúÙ?´ ^'æ?¡Ì_fúØ?îV¹±ž²,?–ØwöŽÏ?ª"dæÝ=?–ØwöŽÏ4FGL J1139.2-6247?ëÇpš?¿ñt¢iKôÀ8†8<‡oËÀ:¿mã2ià@uòœj.r@¸*Ž;?²î	!U©ï?È3<mn˜d@þ¼ž_ç?üQº¥WèÊ¿î¬B®Ûö?ì"ß(#½¿â†¢F†¿áë,i–¿éH§8¾o¿ïþç àö%UNASNone?˜h·ž\÷?žMáä8	?ï<ºGÃ
?žMáä8	?'Ý=Ÿ jX?¬ӝ‰Q1?ïiü­?¬ӝ‰Q2?ώðÇ|ï?´ÙŽ[:+Ä?èCÎ Ä;?´ÙŽ[:+Ã?‹Ûâ"R?|U' ?u²¸?|U' 4FGL J1146.0-0638?àŸîg@JZ?>pÎÀ:b=ç™À<M·½q7@!'Æ¿¬?ùð'Iü?½³TUª?½`OKÔ®?ý\ÄÞÁÂ?þï·]yÙ¿ïý?Æ¿l'?ïAJ·æ¿´|£ÿùõп;«·ShÞ¿Ø-‹¾åƒ}¿ÜŠ"¾@BUNASNone3FGL J1146.1-0640?ïø™pl?Kieè1­¡?M™‹Ò>OÉ?Kieè1­©?ïìß'@;ö?zÔú´f?c Ø¿Ä
Õ?zÔú´g?ïÒ#áqÇ?xˆÀ†RÁ¼?vÿnG'?xˆÀ†RÁº?îQëH{?"PòÿuŽÕ?ªîñK~X]?"PòÿuŽÕ4FGL J1146.0-6822¿¯IMñÖÿXÀ
[>ê÷ZÀ:lF"
qÀ;Àê×yÎù@¾§ðõK@W^ FÇe?ØÖrÓ\3?Õ'H㞠@¿ìTR@ã´2!:b¿ïûì?XÛc?ïÿ©Î›&¿è0Ç}Øró¿â±ŸŒ¨¿ï䍞8º²¿ïÉ™"{UUNASNone?æ?&w?É»§µ×y?Ӂ³ÛÇÓ?É»§µ×y?ëH³uD%?Êð®··?ÂÝ2*ïÿn?Êð®·¶?â</'\?º(#õ'Ø?ۇ ÞÝGÍ?º(#õ'Ø?çšU²õ¯h?¶s^$$?ÐËTš¡/?¶s^$$4FGL J1147.7-6618?ÒV*ŒÀê^ ŸGYÀ9ì¸ô¨´À;{oɼw@ÖÙ¶?A´@…æÿ}ú?ÌÞÏÄ#?Ò6Á}cX@-F|¼A@ç;¸è¿?椔3ÿ
?êÉTýÞ<·¿å'ÊÞ
6æ¿èæRkÞ¿í¡]¹»¿ïüL·h·yUNASNone	?Ñ};ŽYËX?ÆBӈõ¯e?çAb8ÓS?ÆBӈõ¯e?àۙ¼òå%?ÔÿŽ1Œ?ÞH̆5¶?ÔÿŽ1Œ?×EXüGìu?·€i0¡WŒ?ä]SÜ	Å?·€i0¡WŒ?ÊïJ>¥b?°j.-½8X?éD -pV¨?°j.-½8X4FGL J1148.2-0029?ɛºú^î@M<=îx@À;+&ø'MuÀ<‡·ôÎs–@֛3w¦«@BúP"–J?ÆHàÙôþo¿˜à>ˆk?Ñt¶`NÊ=@€èÚ™ô?Æâ=¢Lñu¿Ý"PÄé~‰¿ßÃ!R`¿çúy
2ª¿á\ ý¦‰l¿ïÿå]½JyUNASNone?ïåxØÔi?f€º<ö^?j‡'+ã–Ù?f€º<ö^
?ïøµcEˆã?i*Èò–­?M*réÜpB?i*Èò–­?ï]ÿ[í…y?Œt¶eh(?"@'OPç?Œt¶eh%?ï½ ÚÏ x?j	E~˜â?€—ÉLâ?j	E~˜ä4FGL J1150.1-6324?属S§Ö¿õy€TN5îÀ9·Lz,	À:öðf/	@:Ïzüö`@_¤?åÉ?φbЋž?³Ì{O,8?ð_zNz·V?úH'ëÕ|¿îóÑôSúS?îc2Õ?b¿ãå˜u­+G¿ìbXŸÔF>¿ÛÈFøã¿Ò…(€nzUNASNone?îRjí÷¬ú?°¾Ë~ðU?ªÙQ …0[?°¾Ë~ðU?ꨦµ-ÛZ?І¥!.y?Å]e+H'›?І¥!.y?é"**d?·h7¹[)?Ë¿wWW'p?·h7¹[)?èIJèŇ?¸öÜ –kË?ÎÚÔ\éãŽ?¸öÜ –kË4FGL J1150.7-4613¿ïñVÁ€€É@.ºp6ÉÁÀ:†Æ÷ µîÀ<i´g{9\@›Ö_ȓ@"i7Ñþ?Â&Œš?¸[GàzÏ?÷êg²–À¡?ú%[Øï?ïôÿ¼
aè¿åÊsbοãîð®Se¿Ýñ^|¿åƒ^)+¿ïÿÅbu@UNASNone?ïìŒs	'?eªO=¾º?csŒöâÙ,?eªO=¾¹?íàÂ.hq?½WðøYB?³ùw?½WðøYA?ï¹ãõÐo?Û¥Ûs¡O?‡‹ä;Î?Û¥Ûs¡L?ëãù"È?¢½Êøf±?Àptß÷ß?¢½Êøf±4FGL J1150.8-1905?âÄÅÝ%Ã@DÁâCV—À;Çj
_ÕSÀ<Ýû@ý @"B;ë¾'?õò…=Ân?Ùõð"?Þ¥*ÜÍuê@Ðkæ'ø?ù	E0‹¹¿ïÿ+YJ1?ï)·¿Ža¿ï±	b¦é?ïþmÄ(¹]¿å¥;X›¢ˆ¿ÚD÷€Õ}uUNASNone?ïá€mŒè?n";IhøŠ?n'sqÑ?n";Ihø?îÔýac&°?¼@Û½Ô?¢°)é͕?¼@Û½Ô?ï[HÕ¾®Ý?Ž¾$uvx?"–åH*$Z?Ž¾$uvx?íÿßßµ?¨Ð&a)"?°ISœ?¨Ð&a)"4FGL J1153.7+1857¿îAÞÀÜX@R›ÓíR~RÀ;QÓq+¼FÀ<¦?|ÑÔ@\GŠ®@²9{Kй?Òx‰éù-~?Ãyç!·µ¹?ñJÀ²¤@Gz½áM¿ïÿ*LÚ¤&?ïâ¤.™p¿á¯ÊÈæŽ?¿âzó¼$ÞÝ¿ë6#það5¿ïÍ	žs`UNASNone?ï×ð¢¡+ø?uý:\˜»?t®¯j+?uý:\˜º?ïú%abTv?ahPúÎÚp?Gjzv®(??ahPúÎÚp?î靥ëß?•âî͜±?¡ov%¡B?•âî͜±?ïŽ_À6g?~?¯mÙÓ?Œhòf=ß?~?¯mÙÓ4FGL J1154.5-5952?ë']
°˜å@ÀµgUy¯À9ۅèÜÎÀ;gcRµ¯@íp¨‰¡@¶*ä°a?Ê«r«fÌ?ÞÅè¬ý#­@Â¥Fv@Ñ)÷öP?ïÿ«|,Ò¿ß¼ R:Š¿æ3ªïê¿í'›h¦²‡¿äϵù¿ïQ(l/ÔUNASNone?ãºs[ó®ô?ËÑÖÈp»H?؋H¢?ËÑÖÈp»G?Ó>|âûË?ÓG_»ÅÏ?æ`Áþ'?ÓG_»ÅÏ?Û.O¦ù`¼?»Öÿŀó?âhØ,ƒO¢?»Öÿŀó?ÓÀç×Ûƒ?¶2öa.ç?æŒ{¾?¶2öa.ç4FGL J1155.2-1111?ÕOÇÿÀè
@Hª›(ÂÀ;	)ÿ­ËÀ<ˆ‹y¢ƒ@!õäs2?øRñ>œ?ÜXiwÿk?ÔaæÕw–?ù‰,£Ìù@lƒ¼7©:?Æ5èDL‹?í•9î8W_¿âãeூº¿Ð`LpñÛ¿ÝÓ]ÀOâ¿æßÛÒú
xUNASNone3FGL J1155.3-1112?ï×튜ª?uÄ<b§ÿ9?t	}º±ªã?uÄ<b§ÿ8?ïøOޘ;?n‰étª×‰?NÀ…Ÿý¼?n‰étª×?ï¼ûÿú©º?€"äìò?€ÁU'h?€"äìò?ïnüîw[?}+ÎéÓN?' '1¤?}+ÎéÓO4FGL J1157.7-6327¿¸Þ8Pšò¿óQÚ7ïZ–À8ô".E©À:•,oʓ7@>8?6¡¨@ÏKaþ!Ù?ɔš×1T·?֊MÌ;­U@áã!¢ç÷@÷ÚE±:?ìÚã{dû,?½ê2S¿ç×Tz«—É¿ëb)ösD¿îBýûÈä¿ðUNASNone?¶øžZ»?Ãϟߐ?í ì4¾è ?Ãϟߐ?º¦•d³t¶?ƶˆsi?ì«-Si'i?ƶˆsj?ÆP¢ê"ZÉ?²òV¨™v?êk×EwiN?²òV¨™v?"b`µ?bà€"?ï_ììúX?bà€"4FGL J1158.8-1430?îº;¢ºt@G:‰ãC0×À;ÊNmK]À<}ª?K@!ˆ~7éPf?þ±ÞŸ]'ù?ÁŸ¡EŠx¿¿®å;µg?ïèÞ%d¾?í·«^×À‹?Ô}ÖÅt÷?|¹H­æ$.¿èqԞ}Y¿æ(ŠbÄñ¿Ê"Î×Ë®¿…Ôª'¹{aUNASNone?ïó›Œ-‡?`.6÷£o?XÈçѤól?`.6÷£k?î!_"lÉ?Á"ºý6¶®?¯½ê
Ù3z?Á"ºý6¶®?ï¢2!¯H?…ü¶æÜ'?‡sw».0?…ü¶æÜ'?ë"ub–ú?®ÈóY6NL?Á®*u§ ?®ÈóY6NL4FGL J1202.9+5818¿ï™äµ…@L×z_A®÷À;'bþÒÙVÀ<½·ªü˜l@(¶o\@HÿÚpú?ÄÙ»G¿1Y¿›Ï(¿`n?Ñs×þ")ñ@òà¦ÉX?ïøÀÛýÂ8¿ãÚ¥hõX¿éfòH‡X¿îQ•	ÖC?äp@¥½£¿êÚýç÷ËUNASNone?ïþ£W46?0áÈqwd?%ÎŒ¼¢T?0áÈqwq?ïýˆ«V'?M҇>iw?3º§]NÇT?M҇>i?ﺴÒ3ˆ"?XqCêÑ?RËsÚ×?XqCêÓ?ïýὬN?0j'Åuö?0òÞ^?0j'Åv4FGL J1203.4-6145¿Ùˆ#:ö¸?âé*ÁI¶ØÀ9ƒ×Ð6
ÙÀ:Ñ;§uû/@àúãe@Y~™cõ?ËPk'kSá?Ú=Z¾è]¢@½C^#¡Æ@VÒõÜ?ïÿ9œf¿äӟNå@¿åuWСm£¿êUŒáû2¿ïÿÕ%t.¿íýØ=CWnUNASNone?Õ‹èØl?Ê)äTŒ?å~:"Éü?Ê)äTŒ?Â@?œ"?Ë´ˆã¤e?ëoð9ØÞÿ?Ë´ˆã¤e?Ĺýr¦¼œ?«hÒÉ@€?êр£VPÙ?«hÒÉ@?¥…Á#å7?Ž,Î%BÆ?íÁ¬?Ž,Î%BÇ4FGL J1203.5-1748¿ÖXþ¢=…@E˺Ü	€²À:d&°mñÀ<gÍ0ŸÚü@ý}}":7@…±ã<zÛ?Ȩ|¶^÷1?Ðӛ=]®‡@{ÜpêN@jlU\(¿î³zK¹?ïzV¨ƒAi¿âÍg'ߐõ¿âÁa~õÿK¿î'(]í¿ïÿ•AED®UNASNone3FGL J1203.9-1745?æï"iñC?ÅYë{Ù«t?Ò!»,åz?ÅYë{Ù«t?ëߑ'u¨r?È\'º¼S?À¹º)^9?È\'º¼S?ä²2ýˆç?µ~2üC?×ěšî1?µ~2üC?ãhËp1?ºF¦÷iu@?ÙÇ.ié?ºF¦÷iuA4FGL J1203.5-5745?ÔR"¢E§i@"!Š"CÀ:˜Ž:À;Ö©n"óJ@aÎQ1@ ;êŠ?ÛÓuþ‰Þ;?àÈðÔéÑÀ@YcˆÕý?ü%͌Fµ?ïøÕ~Í"?Þ0×Cÿ¿çcvÇÝyÿé·R²T{'¿ïýðƧÞ?ïâÆ3U—âUNASNone?â‹•¢é?ÐEîíÛ?ÛÒèÔº-Ü?ÐEîíÛ?Î_€Ù¤ã`?ÑFü`:Æ»?èhɖÇ)?ÑFü`:Æ»?ُ§µ‹RB?·Vê¯x¾á?ã8,%:Vß?·Vê¯x¾á?¯7?4ޝj? ˆmá.û?îŒ²)? ˆmá.û4FGL J1203.9-6242¿ã
ôu¾[I¿Õ£òfa´À7럓®žÀ:ƒÝ ×æÜ@åÈøן@lû@}ž'?«uPºÃú?Õå@Ìxé÷@(0ítA@ÁÊqRӍ?îc'ŸÐ¿Õ†šË'¿áW›ÝÁ'°¿æHiü¿ìòFñ'¿ïÿúVrÓ\UNASNone3FGL J1203.9-6243?L'¯œÊ?D"FO»?ïøÿþ[T?D"FO»?[éåˆZ?fî)&ê­6?ïò{ð
;?fî)&ê­6?ƒ¡ìÞÆ^V?qHJe7?ï±xL"æ‡?qHJeE>ñ‹®â,¬>ë	<vA?ïÿÜè¢;Ö>ë	<vA4FGL J1204.3-6111¿Ù'©Ø+?ò¬š'^ÛÀ9Ù¨g'¶QÀ;(Ag©]@úhýoî@悀x`?ԐY—Œy?àœ<ÁÒGá@
ƒn´é?þÀøãÖÿ?ß{ûú?ƒ`MŒiŸ¿çÒ(ÁÀ)P¿í[ˆêዿè.]@L÷*¿ïÿÖDDÓoUNASNone?¹\3Oêûo?Àp8õ_€?ìÔy– '?Àp8õ_€?Ãñ^+·×L?ÍÛ
ñ•‹‹?ë¨u
-?ÍÛ
ñ•‹‹?ËFOe}—?º—êÜ9?é.l:¦ ›?º—êÜ8? ¸\n)V?'
/Jœ§\?îôú9j?'
/Jœ§\4FGL J1204.5-5032?ï󱂇ë¯@'Eík¨Å‡À:]4=õ.À<ˆ໗@æKùӖ@œ…Ý$3?Æ4¸Œ£è?èΙ«7@ Ù#¯2@cLÝ(d£?ïìQ'(¹³¿Ô–)ÂÇt¿ÉôuˆBYA¿è_[5z`¿ïùΝ²X¿ïí¦–Ø:UNASNone?¢@r á6ü?±žQ¼!Ä
?îÛøÝñì?±žQ¼!Ä
?‡Ï<1/+Š?›b—Ÿíwz?ï Ã;CR?›b—Ÿíwy?´¬‹†qyÓ?¤}>ä‡?íjn1ÐÇ?¤}>ä†?ŒØÏÏN?w\þ~GU?ÀÂNj?w\þ~GU4FGL J1205.1-5951¿ÐJ¼N¨4»@ü¢¢&0À:1š‰ƒ¡áÀ;œz'
‹@°†ðõv@…õ'^éš?Ç7ªÉlÆ?ª3¤r:¯ÿ?漺Ñ!Æ#@‹9&A³¿âîO~mnB?ïøYþyC¿èˆV{6Ø¿â­RH¢0A¿í/†ÖHv'?Òja}ss?UNASNone?ìžyUp¬ª?´|ìðd?»5Tzš­?´|ìðe?ì­©qºÌ?Ê7×çÖ?º'´w') ?Ê7×çÖ?ëÀ!ù®¶Ó?ª¢_`´]?ÀÿxE$¶?ª¢_`´_?îLKÜ·Ts?œ
R^b4?«;B4Š¸Ý?œ
R^b44FGL J1206.8-6038c¿âF`‰í™?ü4xã@¬˜À9ÌAƆbÀ;%ÿÜđ•@Êæ¼7(`@.ùèŽÊ?ÐÒíÌw?Ï`Š™ÌoZ@¹5v'\@qæOx?ì¿-b
翱ɫ/C9'¿èöĝSb~¿ä¶‡æ鯿ð?ﶞaUNASNone ?äSr¾ñð±?É°~xFÞ?×Y'ž?É°~xFÞ?ÚÃùʹu?Ւށä'?âú£F?Ւށä'?ڏ¿RŽ4|?·›Yªå ¥?⸠V¸åÃ?·›Yªå ¦?Ód˜/ݼV?»£i̒òÂ?æM³è!Õ?»£i̒òÂ4FGL J1206.8-5836¿ÐiÈCÇÀp@…`&±EÀ:»™ž¢À;ØA'è|V@ê×yÎù@I¥ë·sŸ?ÕÙ*ÞÐÛO?é›ü_âhÀ@¥º9LR@YCNa?ïôáÙú2¿ß1É~X¿å~®@ð‹¿ï!ÃÔֆŠ¿Õ=ŠÅ@fx¿ïþÿðÇôUNASNone	?î_OͶÄ1?²~öFšÇA?ª$"¼ò?²~öFšÇA?Ü¥Ž|HÛñ?֍kc?á­8Áے?֍kc?åpZeB+?·*ÞAý"Ì?ÕK5Ë{ª?·*ÞAý"Ì?â"Ÿ-‹q?Ã^ô
J:?ÛâöÁ¤é?Ã^ô
J:4FGL J1207.4-1840?큮¶!§»@E}NÂò®À;@Ë]a'À<˜Šï²ªã@'¢ivç?þ¦êjl…d?ÓÒÆáÑ@Ð?ВôÏJU?ýkؖ.«@(*…È¿ïüþX`f?ïü1©Æ7‡¿ÙÓåŐ¿æ{°&äp¿ÙÿÛíÒ¿ïÿõEq#UNASNone?ïý†ÊkYa?8÷Ÿ\#^Œ?3ɬ¥4ñÔ?8÷Ÿ\#^–?ïû±ºB6?Z ,Eß±?A9ö%}?Z ,Eߧ?ïe¼§ÿäu?Šã~æy¦?"Hkqb?Šã~æy§?ïÃáݾb¢?m$Ð¥ˆR?~ ήÿ?m$Ð¥ˆR4FGL J1207.4-4536?í͂ùRí,@0"süPHÀ:tŽ·¾GÏÀ<}MPëªÞ@`Tßd?ÿ<¼æ¥¼?Æt~A¤e%?á7^3'þ@#¥ ¶Xí?ñš0Å´Ö?ïÛi³"Ü¿Úï
Kšˆ¿ÎÊ.·Îbú¿æŒ x°ì¿ïÿ
A1"¸?ÊĦ}ìUNASNone3FGL J1207.6-4537?¥¨Y±¾Òô?¯TzÇ÷ô?î¥zdäÑ?¯TzÇ÷ô?¦eYё?À§Y#ŽÎ?bæîÏ?À§Y#ŽÎ? '?ƒ"=?O'8Ñò?îýŒƼ/?O'8Ñò'?‡þû	èô?{ë0ýÔ?ï Ø_‹?{ë0ýÔ4FGL J1207.9-6443c¿ï¬ͅävÀþ}~°àÀ9ÃÚ#Íd¢À;@+ôzÀ@ü¦¬| @ÍG`ç¡d?ǎ¾^9ò?Û`–ƒ9°Ñ@"yJ@«"6‹­H?ï#BÅwmö¿Ý}M¾NÚ¯¿á~@Ï~¿åOãm"BJ¿ïÿþÞ÷?íkP`j£ãUNASNone$?¸R)lëÃ?¼Ñh¨óƒ?ìõºÒâˆ?¼Ñh¨ó'?Û»"ÍË9?ÕÕlcºOp?â"5¸c?ÕÕlcºOo?·
«"Š?¦;«î­'?í¼ªŽOo?¦;«î­'?Ôà®\Ó?ºEL©k?åöù¨Ñ˜?ºEL©k4FGL J1208.0-6900¿êŒ"+C•ÀÖ¢?ZˆãÀ9ú¦wÎm·À<åaïa@*AþR*ð@âÛ,!?À9­å×?×ù%ò-/@ÅJ]ò#ž?ü«?#VqQ¿í¯/˜sÿ¬?ßÑ%ʟ¿à¬ÅZèƒâ¿å'¹ñ·é¿ïÿí¡Ā?é7"^6UNASNone3FGL J1208.0-6901?œQ'ìð?¤º@OŒad?ïgÕvÀ™?¤º@OŒad?Á'[¹{?Èހœ{?ë»v)¾!?Èހœ{?™öbÉ?+ü½Þº?ïÃ7øLé?+ü½Þ¸?»¯²€Z8?¦€Œø­?ìŠɯô¸?¦€Œø­4FGL J1208.2+1158¿ïó%§¬í¸@QñŠ '§À;<n—OßÀ<·;÷ýÒÿ@¡è:@g¸Õ¥¹?л›nÛÖ?ÃsÞt$?óèÚI@E¹F]1‰?³õ¯o烿Þà#`"*¿æîÉp!¿Ó(ËÑ$J¿ïÿÿ" 5•?ïÿú@ùDzUNASNone?ïûØT¨˜?C)ôµh_ï?@ŸÒ­]¢?C)ôµh_ê?ïü.•	N?XOØcF?>‹Wµ‹¬?XOØcF?ï•wíÄhX?Š'v;8ý?Š¢Žåéç?Š'v;8þ?ïåGDƒÅÛ?_úƒ4º@?j¸»|:$Z?_úƒ4ºC4FGL J1208.5-5512?¶¯'±"A@­\œ¹À:Š÷mŠGÀ<'8Yã¡%@×XìÖ-@¥Ò! c¸?О#y+æ?Ö½±[­$ç@P—\¨wƒ?þýîþOü˜?îç%pÔ)¿ßg"ÄËL¿åìÏ¡"c¿ÞB(.rý¿îõõO¢Õ'¿ï#'ŸÐ€UNASNone?éÒQѦµs?ÀP·¦q?ȶ¸¹e*5?ÀP·¦q?äs<¯Ó?ÑFù•¸*	?׆¡òYÅ?ÑFù•¸*	?æ¶I'to?µþl¿Œ?ғlÛó%?µþl¿?ä^¤5‹9ø?°DõÔ9?×B·"éŒ?°DõÔ94FGL J1209.2-7635?Ù:Vo
zXÀ+×ÆÚD""À:Ûe¿wy´À<1"óg°@5°!›[;@›Y<²7ö?˚¸Å-ò?­&û#9t?㑺ýíV/@C%<û^?ì³vð!e«¿ÂdŽŠqÞj¿à&}­ªÈ–¿äÜ`ô6ž"¿×€´ÿÄ¿ïθʷH×UNASNone?ïÈÕÇüè?|ÖI qž?{ý•‹°?|ÖI qž?ïð'¬ß>‰?{Ž5²µY–?^ܦA'íÁ?{Ž5²µY—?ï(ýŠ¥ûó?"[Î	÷?šàN«@œ?"[Î	õ?ï¡RÎÑÔ1?rÝeûÛ[?‡«LKŠó¦?rÝeûÛ[4FGL J1209.4-6421c¿ïù™ƒf´¿ý"€Û\²ˆÀ9"$¼wêóÀ:÷bLLà@ÏrÅz%@#_=}9?ѱœÃ,?Æì¿o?ÿˆÑ•‰i¡?þ\3!•{þ¿ïJAl±Ú?ïõºAYç}¿äÔ6þÄÁ'¿ëôÿñ½G¿éÁ2?B`"¿Ùúc
UNASNone8?äÏßÉÞØ?Ì#Tq®·$?Ö`@lBOü?Ì#Tq®·$?æf~ʂø?Ó»ÏÔs?Ó3jûø?Ó»ÏÔs?à×Ùú™Ž?½l1Û|ëJ?ÞPMÞ
Ìã?½l1Û|ëJ?ÚXÎõˆ?À—ã˜ÿ?âӘ…7»þ?À—ã˜ÿ4FGL J1210.1+3241¿ì³ç‡Ú@SÞ\å´$_À;ÅÚ(ÕâÀ<é(kYn@!\tWë¤S?ûYê¦Òg?Ù>4ƒ•KV?¯ô¾®Q¶?Þý-<ÏN?ýíôOG»Ö¿ïþh›Œ¹?ïúµÞs¾>¿â¿Àʶ¿ïsøö ƒ?î0?)á{¿ïÿ¸GʐUNASNone?ï÷cÛðç? .¤Oãú¶?Pý8H2h? .¤Oãú¶?ïü×,µa¼?U/Ÿޚk?9FšTò'?U/Ÿޚn?ïdv ÌK×?Ž½|ܙÂ?"q;æv…?Ž½|ܙÀ?ïöÆaÝý?TMBɝ(?RsÑ<D?TMBɝ-4FGL J1210.4-6250¿ïv·Fxm>¿ÕmÒÁXzjÀ9XsHÍÀ:še"¯O@¦—Ìdòô@ø¶zzða?Ð"Ág	?ëøìæGÈ@s@ªÀ3?ùU®ˆ>(¿ê w~瑟?¼ÚÇ·9<¸¿ÜK¹ý<VH¿îz̺XV¿àŸÑß[E¿ïÿ2Ȫ(UNASNone?»í¥ÖQ?Áæü5y?ìžâKE<v?Áæü5y?«$ËNÓE?À×à­è‡1?îM·#KÌ?À×à­è‡1?ÇÍ4}–²}?¶7|—z¿ê?ê²àšS`?¶7|—z¿ê?T«[Ž»Ó-?Pð¢Øüã?ïõªR8¢?Pð¢Øüã4FGL J1210.4-6100c¿ì™Ïª««þ?÷|…Ý$2åÀ:@ù¬(èWÀ;igI»4õ@ H.}ÁÌ¿@‡åÝ?
Ø?˪µJÐë?²ór}öÑ?íá8ÿûÎB@VÃÉBÿ"¿ëü'§:?ác¢1пÚ*{žÜÏy¿å¬vJßø#¿èÁ‹ ²'¿åWÃ Ô ~UNASNone8?ïTÔÃ^˜Ç?—t}¤ÄeÁ?•eg",ç9?—t}¤ÄeÀ?î†Ï`?Áàè¶&ñ?§ŸƒÉ÷%?Áàè¶&ñ?ì¬"eÙ?­9Þ¦vTm?ºžì×Ç;?­9Þ¦vTl?ïs%Œ	?ƒº"p.žo?'›N}~>õ?ƒº"p.žo4FGL J1210.7-6005c¿êÆfãם-@	1*À:n+ë†ÌÀ;k*þ±K@ 	ÃÑ%¡û@të<#œ½?Õ[H{úù?ÆLCe'Š?÷&q3I¨@$lÆÒ¸¿ïøcß"Í?ïÿvmD¦ù¿çQÁÚM¿æÂ:½k/ú¿áFmlêäæ¿çp$ sRˆUNASNone8?îÝefÍ|;?¦žåSÎ<å?¢)©"(<L?¦žåSÎ<æ?æ\€b›m?Õ·´+àÝO?ÓGÿ:É'?Õ·´+àÝP?鬱w<‹?¸RGÛ¾i€?ÉM;Î#
Ö?¸RGÛ¾i€?î*ÚdÌ&(?¡WRŠ
Õ?­RY³=?¡WRŠ
Õ4FGL J1213.1-5957¿î•@…o˜@ø¨ó©°À:Ç"hà"À;²þ¾·`T@Wÿ¡`bk@ށËFºÏ?Հ"ûOA1?ãÇkcü(Û@F{åS¬?üü‰Ñ$ H¿ï÷fÁ1
?ïúõ—k¿á£8I©"¿ä\«!Vfê¿ïþæŜVã¿ßëXZ4)UNASNone?µÀ¿›¥!\?»ø©"=}ÿ?íGè‹[Õ?»ø©"=}ÿ?¢Â#.zú‹?°B•¼nd?îÓÝÍPX?°B•¼nd?Ãø!›psH?¯èUc˜?ë÷™#ã-?¯èUc˜?«TŬã¬ô?–:±q¬"?îJ³¥1Å1?–:±q¬"4FGL J1213.9-4416?ê·¿T8€@2b€'،À9ÿ'xë¤(À;÷%=§*|@c®%AÙ@[¹™ê!q?¼b?PÍÎ?ÍhŽŸ? Õ@m.¼«íY@aBŽ?ï»|þX`?ğÚ{aU¿åZ³uòW¿ãû}å3 ¿ëmª]6;ü¿îlЮÝ*UNASNone3FGL J1213.9-4412?=®^®R?"ôe`?ï~
¦?"ôe`?°pZz¨Ê†?º{ô¡Ÿiï?íñô°ªæ°?º{ô¡Ÿiî?ǹ:Ûè?²Ñ"'d'?ê>±Iü?²Ñ"'d'?ÂóxO¢o!?¥!«N;ì?ëC!ìd7?¥!«N;ì4FGL J1214.5-2318¿ï·Žìôè@Cc‰!S7À:ӕÄ"`À<o]2K­@\Ž´
c@?ýהÁÄO?Ô(ªÄbC?Ñ.…dˆñ?ÿÏ'T·@øSK+¢p¿ÕC	ËÜ?ê#X)ŒÁD¿Ó¬¡«¶Ó¿ÞӎóMj¿äøSδ-š¿ïÿ7¸Óñ"UNASNone3FGL J1214.4-2315?ïû¢y"<?@⽗M5?Avïå?@⽗M??ïû")àŒ?[ªüœqGÆ?A³»X}Ð
?[ªüœqG¿?ï¡zµ"?"\1vgN?‡¡{¼Zò?"\1vgN?ï·bŠJ ?n6礠?'']xíXR?n6礞4FGL J1214.7-5858¿ï
Š¯Ä=@'Ä$#À9¦`;©ú:À;kT/,=v@ÛÌ{O,@-¦¿
"?ÈïcЉð¯?ÁÏ+KÞ$ä?þ<xVRòì@•€ZXf?ËM¹Ü°¹¿½håq´MO¿é^´ás¢å¿æ1neZοïÿs³VB?ï¾h…ûW$UNASNone?êTúæWõ?çï|îg?Ƭf +º?çï|îg?啥r¿Ð?Ó%~4
D?ÔÔµ΀_?Ó%~4
E?èMoôþÏ?µnl7Ó?ÎÊ@/¤Á?µnl7Ò?ç¶c°ˆâB?¶£OÕ¦ÀÐ?Г8žî;}?¶£OÕ¦ÀÐ4FGL J1216.2+0537¿ìeCÂa´@P»>-b9À;}JØkf€À<¶]ŠÒS@ R"²,?ÿ«cÆxö?ÕV¶JªH?Σ€ùÊ?êžwïû¥þ@	&'=TŸ??¯®Ï¶·Å?¨Ã=ë¨¿ÔÝç®Ðc¿åÕuþ3÷ÿ¿Ü4ÄØ·'¿ìÐ=ÊeêUNASNone?ï÷‰áÃ?Oç ½1þý?Pì<áðy
?Oç ½1þö?ïýEá™Øi?O5õ¡m¿?5Ðó1<µ?O5õ¡m»?ïjJ«'1?‹ow°7§?'¶ª½9Í?‹ow°7§?ïò¿FÎS1?JðÏ7¯1µ?ZrcYŸP?JðÏ7¯1´4FGL J1216.2-0600¿ËÈ-Þ<MÓ@Kå2µ^ñþÀ9ÈÏuôxãÀ<,νgÔû@¸™nÑnó@—¯ê=öÜ?¸óÓÌÆAÃ?½Té;mie?þ±Á
{é…@D,²™Æ¿àsûz_B¿âž.>VÒ˿蟦=ìʙ¿âtŒ>'6ú¿ï¿¸Så¿ðUNASNone3FGL J1216.6-0557?îçx\•M!? õä»^§?¡ˆz6«.? õä»^§?î°æÝû=?¶25šY¥?¤ñŸÂ L'?¶25šY¥?í'í%öĘ?£7îT| ¢?³p–ÐIÛG?£7îT| ¢?êÒ`KRpÏ?­ñ9®>¸C?Ķ~Ò¶<Ç?­ñ9®>¸C4FGL J1216.2-1550¿²TBóó» @G5ü;OaÀ;W%­AíÀ<šÖvš@ JB¾@
¤‡3f?Оi¢…üY?®®£Áæ"Ê?߸©)Y•ž?÷¼"*F¦?æáJ2S9¿ÕãvÇÝyÿԒ/BêÊ¿çÚ\FQô?—˜×…k¿ïðÃhŸýUNASNone?ïôÌ^ï	þ?]Em»'÷s?VgB!ìÏ?]Em»'÷}?ïöâ'•/?k­w'R¿?R:ûàÕ¡j?k­w'R½?ï'Îé«Oq?†ÇƒçÈ?‹ŒE•,#î?†ÇƒçÄ?ïW=dàh?€ÿdÐ)æ?ª0¦Çåø?€ÿdÐ)ç4FGL J1216.4-1358?ÚHqL"Ëb@HŸU›=À;&:Wê£À<…AøDJ@ [&¤«@5ºÚ\‰?Å}®ˆ*Ü¿|8ù" Ðý?¶POx¹$N@<€;¤›Ö¿ï·1Å?ï îؐO?ÎH»…§ŸA¿çviéпïø£NNB?ï인KhUNASNone?ïüÆJ'/Ã?<âü'Ú?9Í«îé²?<âü'Ë?ïýcmr`?RAhÿ½?4ç<"lüö?RAhÿ³?ïklÛ{—?"
ºýCþ?R'd,?"
ºýCý?ïðÔPj1[?Y´/w?^W_+Hy?Y´/s4FGL J1216.8-5955¿ïžB®—P@>ØÓkLÀ9bsýþžÀ;%‡\€3—@/ÛåÄj@¾S<½öp?À愙WT{?Ï{£ºY؎@9[Ývh<@èÀr×
?áRá"öW¿áôÁÞ\A¿è9Xç!â©¿æZÙ㐿îgñ`ªåœ¿ïåaHÌ"UNASNone?§uÕÍ]n?¨æûÆÇ}t?£.º)?¨æûÆÇ}u?¯Êÿ=Þ+?¿fE0'%š?îPL"?¿fE0'%š?ÎÇÉÉJÔ?²')8´	»?èN
¾mK?²')8´	¼?³»9\usd?˜…FÃE0?툘ÔqQ"?˜…FÃE14FGL J1217.2-2500¿àQÖsjíŠ@B›ÿñÀ;k$á`؈À<Ô¯«SÖA@¶E‰÷æ@>¢'vge?ØfÜ­ë`6?æ—r½·±@
›©ÄŠ,?üüøÔg Î¿èPä>X€J¿á Îï¼¼¿›à®^«9³¿ãêv–_Rv¿ïÿà•V"¿ïÁa)ÃÂUNASNone?ä¿lÔèL?Çù#ŸœI?×à&V/h?Çù#ŸœI?ä$Z×Öƒ?сÜhu¥Ÿ?×·JPSØù?сÜhu¥Ÿ?åýáÀØ)V?·ß1ö¢xŽ?Ô<~O­T?·ß1ö¢xŽ?Õ÷üÏ®Qe?³gÀ5+=È?å˜(×N?³gÀ5+=È4FGL J1218.6-1049?á°ò@òÍ%@Iœ,ÂãÀ:´'QžXÀ<L#{/KG@ؓ…ƒb @ßoijù—?Ӑ¡7óŒT?á6,­4¨@ó÷ ]m™@áÞõnW?ïÿ·hª¿Û'{°)©¿éhÚ´ìÜ7¿ð?ïú—á2µ_?ïÿ¢bôUNASNone?ïþjŤf?:•msãÝ?)_󥹜o?:•msãð?ïô'¨Í[¹?}þ°5­Ÿ+?Vú®eHŽ?}þ°5­Ÿ-?í,þ€+ų?£-¸-–¶j?¶˜þ¡Òb?£-¸-–¶k?ïîî,sv?f-Ø Ü4?aӌéŠ+?f-Ø Ü44FGL J1220.1-5558¿ïåFMhl6@ŠŒ›"UeÀ9é'Dé>À;î(«ð´3@ßG`'»)@µ'-lJ?Ã+þ +ïr?ţܾ‡d¹@Á\ºT$@tÔHD:?調.%­¿äëEÉ7ìÖ¿àÒÿ¡‹U‰¿å(‹¤äPw¿ï±‡¿g¿ïýyb—yÚUNASNone?î[Dã]AB?©S"ÍIžã?ªK±Ê+ëá?©S"ÍIžã?ï	ތBJ¶?²6)Ãu.:?žÄ.w¶©B?²6)Ãu.:?í$ç´@?¤öJ2£ÆŽ?¶ØÂ]ÿk‹?¤öJ2£Æ?í*˜¥©R?š´ãÑ¡!'?¶«:Ò·5q?š´ãÑ¡!'4FGL J1220.1-2458?ÑdêývN@B­³Ð|"¶À:œ€šÅÀ<c«Ø`~Æ@ _ºª@TXÍ ¯£?ÀmÓÃ-¿‡<3•ŒL]?Ȭ| 9›Ø@Iۂr6?ë|¿€^	¿ä)ôÆ)¿â<½ ‰ø½¿ÜB_ !¿á¡–
W¿ÕM!ñÂO›UNASNone3FGL J1220.0-2502?ï¯?Wó3^åy?`sPðíQ:?Wó3^åy"?ïý‰þâôL?LùVµËÂ?3°è]ŸZ?LùVµËÁ?ï÷­>ØV©?\åžKÜb?P¥'OR®?\åžKÜY?ïÛ65ºC?YæœQh*ÿ?rdå"ü^ç?YæœQh*ù4FGL J1220.5-2745?èûYu²½D@AMçê_"ËÀ:zÉۀĶÀ<>ðd‰Ø@wQ-=¿@¨tBÇû­?ĕeTB¢?¶Ñb?ïf þ'@Iòµ>»¨¿é­ûPm׿Þ†nCªz¿ìbÁì!¿Û"fy±œÆ¿ìÿ»Ëǔ¿ïÿ\l¡UNASNone?ï°oŒ'/¥?…'è™?ƒäö4Ì?…'è™?ïÛÚYäå?Œ¡$K?rÓ
tx?Œ¡$K~?ï1 ·é7?'bþ™ê¬ž?™ËüÉÙ?'bþ™ê¬?ï‡>šŽš}?|u
»C¾?Ž0Y\Y`®?|u
»C¼4FGL J1224.6+7011?êõCÜ|@GaFÜ]cˆÀ:\H»Z´À<PÑæAq@ ­'ÐÅ@7ºœH ƒ?¹Ð­'ÐÅ¿¡ÊžÕ˜£?ââuuÍâw@]/ÆO?ïÿ
¢q›¿æFIlÊ.¿ë ²Ý¸Wu¿å¸
ñâ¿ã8?!(οïÿøþÙå9UNASNone?ïú²Fir ?Z3¥Nûì?E6æZ5c?Z3¥Nûì?ïäºû^\?‡`‡JŸ¿±?kâE¡£×?‡`‡JŸ¿±?ï£Bzò?"L'S+Mÿ?‡/a~ÿÇ?"L'S+N?ªTã?{(úò›ÍK?Š'Õjú†Õ?{(úò›ÍK4FGL J1225.9+2951¿ïê/Ÿ‡@Tñw[0À9'7 þ}IÀ<@̺XV@±È,)(Ã?üT¤MQÂ?·JRŸ	E#?Ú÷FóÚWÐ@"Ðàm"@±a5$$"?ï•¿,{3?ÌïÒ Ì=Ü¿ÑPLH­î»¿ÝΌ 6즿í]¨QÃA¿ïêo_‰RzUNASNone3FGL J1225.9+2953?qHJE¶ÃR?Ÿ  ™Ì¹·?ïÝokt'z?Ÿ  ™Ì¹¸?¦œŒ'ƒð&?½¬¤zfß?î–7=‡Àþ?½¬¤zfß?¤mÅu ÂÊ?œnË^Ÿê¿?î¹#¨­óÓ?œnË^Ÿê¾?N愐Y+?Ct×Ó|%?ïøF^Ûéµ?Ct×Ó|%4FGL J1226.5+3023¿•ªÃµ"@TéªÍžƒäÀ;A§
›duÀ<x
c0Q@S͍'ùg@ÁòÜ+¢?Ì¡›†-Öþ?™]g—Çe?È01¡Õ{@#r ÜY¿ë^¿¨÷Ûn¿ÙhòÝ­š­¿Ø@ãȑտëÞ
Â5o#? æPž`~¿ïÿ›¡[¯ÔUNASNone?ïñ˜H^É?]XmºO%?\ÏoCØmj?]XmºO$?ïýVþ¸R—?Q}—Ï-µƒ?5H
=kI–?Q}—Ï-µƒ?ïmh 1œ?Œ˜L+¥/?'Rûùߌ'?Œ˜L+¥0?ïñüŒ½R?T<O cü?]Èæ…ZÓ?T<O cü4FGL J1226.8-4907¿î}+5Ö@+ÄÞÁÁ×À9}ÎéöÀ;PÜ¢b–@	ÛhQx@B Ž€a?¾ß¡:ͱ?Ç=ýçvò%@H™|=h@@
EBÉ(R…¿íóû¶Å?ÎâüúgØ¿êO"J'°¿î«ØáX&¿ïú	.Îõ?ïá c¸6=UNASNone?ïïÀuý\5?pUr–ú}?`?Š£ÊÑ?pUr–ú~?ïH'?·ïKàϨ?öü[1?·ïKàϨ?Ꚓ±7W1?®Î'ÎÒwô?ŕµ;"£<?®Î'ÎÒwô?ï~ú«žö—?ƒ'½70Èq? ªŒ!-2?ƒ'½70Èp4FGL J1228.0-6918?ç¢H.¦À#âOëОÀ:ÇM~8DÀ<)©HcF @Ùe4%m@o«Ú
ýð?ËT3]û]Ú?»(‰Œ\`?ð•¢y<,?ý9+€À…?íKT'
`ç¿èÿ §?tŠ¿ä|<& ûù¿ã.÷ϯÖ¿ç…ý_çœ1¿ïŸ€-·É0UNASNone?ï@ڊ?a\­¢ˆ*?aq¿%vf?a\­¢ˆ+?ï'ª7â-?¡'$ÂKÀ?‹¹•rty?¡'$ÂK¿?×Ûú?†¤Þ	+Zv?ŒÕþ
	^?†¤Þ	+Zs?îJ}=M?¥9ôþ…?«^è,+.'?¥9ôþ…4FGL J1229.5-3048¿ßzźk@?Ó ù	kºÀ:óD{ZrÀ<e†Üþs@âƌì¸@»œ"á?ÖØ­Áä}?ÉäbÈ!?õH(¨•µß?ú`ŒzLL_¿Þ)Q¨,Y¿êR½<6¿Ûœ²þšz?¿çEa-¡¿î	‡"s\¿ïêvUNASNone?ïN_E¢9?"…X… ½?–4WK¸Ò?"…X… ½?ïQÓb•?¥2"I£î?•ÅŸ"­^Ü?¥2"I£î?ìЎ(zzÁ?£öjCPg?¹{Ž¼,)ö?£öjCPg?í'r₶Ë?4ù1PÌ?¶ÄhëêI¨?4ù1PÍ4FGL J1231.6-5116¿Ïe½¦¯@&÷\òI^À9ZZ¦>ÊÀ<z>ŠJ@F:ωÀ‰@fû_‡O?¸4€·å#?æj'ào–ç@'•€^_0è@¾€JGÖ?ïÈÜ}Cø}¿½Þ½åÿ"à¿äw݇/3Ê¿ïi'2t¿ð?ðUNASNone3FGL J1231.6-5113?µ¶⏋?¨ΚÍu?íI=C®?¨ΚÍu?€g³!"Ö\?ªz è?ï¾a3{t§?ªz è?ƆšÐ~80?±¤")pG
?ê^YKàqô?±¤")pG
?Љ¸­P?qӉ?ïÿ9{²:"?qӉ4FGL J1231.6-6511?çÀ­Ó£«À6Ÿ~µè…À96‰@†
À;9åèý"û@ٝÃõ¸©@"dEú¶?Ân D2Ò?ÝÊBÄJÈ%@ɝ_÷·\?ÿ'—¿ïÿÿ)@k*?ïÿþˆ0»Š¿à¿"àT¾ô¿êŒ@À}¿ìý¢yM¿ïûîיåUNASNone3FGL J1231.7-6513?™Ò]ú=s?²E+Š‡cC?ï1m/n?²E+Š‡cC?£Kö‡G½?¹Öe]U?îË@—Û…?¹Öe]U?°ÿéJͤ?¢•'Âsr?íàÖ¼¦L?¢•'Âsq?VLÝuQÏ?o¡¹Ã³Þ|?ﺦ̊*¸?o¡¹Ã³Þ}4FGL J1231.7-6653?ꈛ¥`ЂÀcËďªÀ9ðh¬'ÃâÀ;G¸ü5p$@ÕúK`%°@¥EŸF'?Ô͍Ý"ÛL?ãÂÜSRl@	ôŽ:!d@!$‰w7š?ÚþcGοågÔôó¿ì®Êžc˜¿ëiäñÒÁ¿ð?ïþ× ¿UNASNone?ížÜ>pr?¼à#þ}J?³	|r?¼à#þ}J?å=Ã,IÓ?Ô]4| Ò?Ô߄y§l[?Ô]4| Ò?ã*ô»s?µü'Õü?ÙÉ᪉?µü'Õü?Ց<»Ä9†?À0]êæ´F?å7a¢ã<?À0]êæ´F4FGL J1232.1+5953¿ÄMÐ+ű¼@L‰ÄڐïÀ;½—¥¤À<³Ùý7@õH&4r#@	=·ä{õ?ÊÈü]´¿®RºÀŽX¦?ÜüϞä1B@v=}dá¿ð?ð¿í9~¦Ï¿ïÄ_@¿ï0_y[X?ïGâ¢w
ÓUNASNone?ïþÎ}ëz?QÝ".?#!H^r—?QÝ".?ï`"
ÕVL?¬O˜™÷?"í~¥U6"?¬O˜™÷?îZ(š¡!?š•ê§î&´?ª_­vUíõ?š•ê§î&µ?ï£ýðéø?ðƒ'ürŽ?‡ƒø'?ðƒ'ür4FGL J1233.0+1333¿ÁVUк^î@RðÞÑ·À:ü˜lrðÀ<B½=ã^@&Ø,ý9&@§ …±…I?Ãd´ CŒ?Ìf7AŠ¹Ø@ä†&ö@Õîßq??ïóçÞ¡
§¿ÖŠîü!¤¿åß«Ì¢¢¿èH'_ì#տ뒥2.¿ïñ">¿UNASNone3FGL J1232.8+1332?îTÕ4¯‹m?§D
Cl†?ª²¬µI-?§D
Cl†?³‡mŸ?¯‰aý¬w?Ž^Ó$˜d?¯‰aý¬v?ëb*Pªý…?ªÑþ±î÷Ã?ÂwV½T	é?ªÑþ±î÷Ã?ëz!Ü÷ö?¥õ–²b×6?ÂxŒ#Ä*?¥õ–²b×64FGL J1239.7-3455?ȵìx5Çú@;âbS—À:ÐDñ¡˜lÀ<Bãü";@äÊ-
O9@%1"Éÿ?Àq2GOõ·¿³d$í ,?ñËý™ô2@Y±=¥'?Ò
»Då_¿æ¦F…öN¦¿ïÿô¬å¦¸?ïýŸêÁ¿Ñüê
î¿íIhÉíõ<UNASNone?ïñI9†Âå?[sgM9\Ñ?]mŒòz5ª?[sgM9\Ç?ïüìž]µ¬?gB»‡
ô+?8›
R›Ë?gB»‡
ô,?ïÆêz1ÜÑ?}'	x<'?|ŠÂç—<?}'	x<,?ïüÜ,Ú"??NµíyÍA?9™/6ìQ??NµíyÍI4FGL J1243.5+5311?ïûОÊU@Oñ\(öÀ;´vTðóÀ=C'üÇf@ cõpÚވ?þ*(,nô?ÔªL¤ô@¯?±Ž%È¥j?ÞzÊáæ'@x8֋<Š¿ë$ñ`®—¿ì.û€"dü¿µ™ÆÿÈ"¿Ô*¡OÆ¿ïx×ì;?ìÄs'-Â0UNASNone?ïÿhµÞVj?Pì¯RÂÜ?éD52ª²?Pì¯RÂñ?ïý®"•?Kì6
8k?2‹gSW(?Kì6
8k!?ïwû"P«?a»p©¡=?'}uê¦?a»p©¡9?ïú""­ùµ?>E&†lÕ'?EïuH,ƒ?>E&†lÕ\4FGL J1243.7+1727¿ïèjÀÃ@T
¯%;À;9@À<Ù$H¸@ ‡Z$ää@\ú&¢+9?Å´ØÏå[¿¶9÷GŸ¦Ï?壼gú»?ù"€€Ce¿çGìþ›{ò¿ìDåýö:"¿Þ5'm,S¿Ø쮿p˜Ä¿×`^l¢¿åIÛ¶t›³UNASNone?ïù?˼?E®X]b—ï?K"ÑÅ?E®X]b—þ?ïögÚ"§?pè(ᬨ?S0Kâز*?pè(ᬨ?ïâhÕq1?vÐnÍ,ß?må—*ŽÏM?vÐnÍ,ß?ïœ#'†¼?{+>割?ˆ÷^Pø{?{+>剴4FGL J1244.3-6233?ëÉó˜XCš?Ӝ?{Àë˜À8Y®4[Q_À:Žž @7Û@&ªfpwa?¶Ž±3>F?º×Eâz@ÉÉã
€ò?ø8DD}ˆl?ïÓ5!	†¿ÆgÆ£=q¿ãg]Ý*é¿æÞíášdE¿ë›@˜vƒë¿ï.
ß¼"šUNASNone3FGL J1244.2-6227?Ïñ¼¤ˆNÅ?Ç=0]ôî"?èÖÝìN?Ç=0]ôî"?·Tå*…?Æ9"—Êq2?í|#Z¿?Æ9"—Êq2?ÜÍ`îÃ"ž?º³ÈîÑ`?á™Oˆžn±?º³ÈîÑ_? Æ%dÄ?Ž4´·ÞÉo?î󝩳¿¾?Ž4´·ÞÉo4FGL J1250.8-5424?Ó«ey@ î)Ø@žVÀ:ƒø³o.À<Ï<é•Z@¶Nií"@qº?À~ÀzY
?"0'—|<?хX.•>Á@•x´Ðì?ïÿdd-§¿ÖЏ$Äì¿æ8õ³¿Ù¾@Bo	¿éŽÌܽ¿ØˆUg"UNASNone?ï‡ø-·¸?‰·rs0¬?Žô'܄?‰·rs0­?ïô%þüæ?w=­Gv£k?Wó´45?w=­Gv£i?îù REØ??–<RÊj#s? múÛ¢|?–<RÊj#r?ï´$1µÚ??jxL"þÀ?'öó'‰p1?jxL"þÂ4FGL J1250.9-4943?Ô"Îíûå\@*M~Ë·ù×À9ñ¿³ß•ýÀ<8#;nk@'.íÿ"@ÿCB?½jtËáY?¾ÖÜG©ã@Å$aß@iˆZ?ë†+'Ëöä?ÚAžlK¿äÏ?mÔñ¿Ñô" áw¿åˆë–¼o‡¿ë:ÿ[ë8UNASNone3FGL J1251.0-4943?ïåCÕìrS?h_­enïæ?j¼*­V?h_­enïå?ïßñ'–»x?‰2ÕU\?p>´¢DS?‰2ÕU\?ïÍ4s!ä#?|p7NAf??yeÆo
î½?|p7NAf=?ï>°ÅDŽ?€—ù+rº§?˜)ç]·nA?€—ù+rº§4FGL J1252.7-2520¿À~%¬g;P@B»ýq°GÀ:£9Œé‡îÀ;ëô9rè@"<͐Â@RoFøÍ?á¥ô@")›?ÕBTcY–Ÿ?ðèçÖyõ@…ë´½·¿©uy~Çc?áOmŽo¿èM_.cÀš¿ïqKÞ'ñ?ßÎùã0fz¿ïÿüÉï£UNASNone?ï9_RŸ?¬&Lf?œøÝ´¬-?¬&Lg?ïüvp?[7_G/?<OW"C´?[7_G2?ê\´QÑ?°"]2‹T<?ƍ/φ¸º?°"]2‹T<?ïð¢|l'ì?Y‰z<æ?^»'°)–?Y‰z<æ4FGL J1254.7-4516¿×G2¢—aÖ@1—Ö[åÚÀ;…Y#‡Ä…À=gû'@ RTN‹Ô4?÷%
`¬B?Ö¶N›™y
?鎥.i@g›\è8c@ʈˆ¥*œ?ïÿá'¢±¿íä‡imP?܄",tþ¿¿)¤i+g¸¿èý0½b ±¿ïÿýawUNASNone?ï£=Œ_‹¨?ŒÿÇäÊ¥è?‡0œèã?ŒÿÇäÊ¥é?íÆ3Ì·\?²\1Èí?±ÎašE#?²\1Èí?ì@éÂå@Ñ?©~º¾'Ú?½ø±èÕùy?©~º¾'Ú?è¿¥º0Ã?·̟Ó|G?Íi?"ô?·̟Ó|G4FGL J1256.8+5329¿Æ©EíT4@OÏÞ灃ùÀ:A'½µÕÀ<2ºOò†›@¸b4þdt@@'w?¿JriÿÎ?´Å–¶eW?ñ~@'7|n@Ï&ݺZÚ?î!၏·™¿åPʽþÓ°¿ép¿ñ7n¿ä–fr•I¿ïÿ+Žúg?ïæG\µã|UNASNone3FGL J1256.7+5328?ïk³Œ÷+r?"-Fú
³7?'‰Ža'Ï?"-Fú
³7?ï2kVɊš?°Uù±ÉS2?™²•&άå?°Uù±ÉS2?ï%PFS9I?'î]}Rk?›U÷5˜Öç?'î]}Rl?îgšhNm?›?æɋ½k?©†Y{.Ã?›?æɋ½k4FGL J1256.8-1333¿ï?A¹kÏõ@H¥VHþÀ;-Þ5ªÜ¸À<ˆK¹ë@KsÙ@¤@}= t.?Çè£ØaÖ_¿¤—±U±?Üí7OË@ëFƏq¿Ø/›#1ˆ¿Ø‡Ø_ñ¿ëk!ÃI@¿ÄÔèå‡-Ü¿ál‹ä¥0§¿ïúlb~Ð@UNASNone?ïó>ŸH?X¡§ãÔ?YƒÞÁÃp(?X¡§ãÔ?ïüÇór:¼?_K*mytY?9Àdn*´?_K*mytP?ïË hd#?x¶"§?zt/ËÍî¶?x¶"§?ïóD~"˜?K`n"Ÿ­?YwöҔ?K`n"Ÿ±4FGL J1256.9+2736¿ØÓcŒà-»@V+©¨–hÀ;äa1sÀ<£u»mÿ¸@á#õ[â@Š;WÄã?Ѭþüôã?Àå—IZè?èi®ðBô@ïƝޢ¸¿àf» Õx¿Õo"'`í׿ì•C~Yø¿Ô[€–é;¿ïýîþOü˜¿ïóöúUNASNone?ïæ@5ñXù?q(9ªÄî$?i¿Ê§U?q(9ªÄî&?ïç&´¥®?‹o´QQX?hÙKZûR^?‹o´QQX?ï³(¾¾?'
$ÌÎì?œÉšýh(1?'
$ÌÎì?ï›Y²Rì×?~'Õ3è?‰)"kDÊB?~'Õ3è4FGL J1257.0-6339¿ØTbue1²¿éO0«¼²À9=Åté¶èÀ;nããiÇ@8¯ÿ;_@˜«B8‰´?†'vçh?՘" ;^Ñ@
à×ò›?ï,é™BS¿ïýð@o[Ø?ïÁW]ßÚ?¨f]O³¿¿ä-Þ)ìb"¿ê.^¸; ¿îD$QîàUNASNone3FGL J1257.0-6338?µoµì—6?ÀUL½nš‹?íR	BnM?ÀUL½nš‹?µ¥
i:?ÆjrWms?íK^¿Ý²Ù?ÆjrWms?Ë!Ï'd'Ò?²à˜ñG?é7Œ6&ßL?²à˜ñG?>€²á!?ˆ#H·÷Щ?ïÿ
hø?ˆ#H·÷Щ4FGL J1258.4+6554¿çÄÌPùÑ^@IšÏ¿ÆT
À;"åV0Ž=À=%|'K@\P¡X)ã@¾Àdß}©?ÌÍ¢à•+¡?'wÿ&L?Ò%œq».@Æ-Ní¤¿ê˜›î¿âQ–?òß0¿îÛK_ú¼t?çGÍ+¿ìÚǗæd¿ïÿå"m/®UNASNone?ï÷•¸xÑ?Ræ]yû1?PÕЏ]7?Ræ]yû/?ïý<ˆù-?Zôaa±è?7þ¸6˜]?Zôaa±ê?ïŸðë1?ˆBù?ˆø½Å3'?ˆBù
ý?ïûù‹?ó?=›Ðí*‰?@Ó2F?=›Ðí*"4FGL J1258.5-3406¿ïÅúܹõª@<¾š,fXÀ:¥{ 1ίÀ<U /Äê@Æs—Qj×@@D
û?ÅÆ÷ܔ@?£uÌàÃÏ£?Ü0«½@>älP¶¿çž¬ÞšÕ"¿ã¯=šÀ5¿å>#¶e¿Ûa®[G¤Y¿ïúûHáb?ïNž=î"2UNASNone?ïìA¿ÿ
?f+y:ß?c¾b@õ/?f+y:à?ïúDž3®q?s™Ø~;FS?Dáë1F?L?s™Ø~;FR?ï¯PÌ8ž?",Ñ]Œ€þ?"+ÌñûØÑ?",Ñ]Œ€ÿ?ïé×ˤ(¹?[A­'ÿ®ÿ?f(4[×G{?[A­'ÿ¯4FGL J1259.0-8148¿«ò$ü•]ÅÀ2òã'÷ÓÀ:4·b|ØÀ;úÏ®ÿ\l@U-ß6[Ý@1Ze§#Æ?ÄETÈÚ#ø?Ö ÛâêE"@:¤vlmç?ù­q:)òm?ÌÆQ)³¿à*_"ÊÕ|¿ãnO3Cú+¿é°¥ŸaY·¿ïýá!˜¿ímî$nUNASNone3FGL J1259.3-8151?³ßjӗ[å?´jPo˜^×?í"¥ƒ?´jPo˜^×?ϱ}(-ö?Ð۟`l»Ø?è µútƒ?Ð۟`l»Ø?¼ÛµŸ:È?§iÉñ<Sø?ìd‰L§?§iÉñ<Sù?¾h¬ß˜P? ²hÐZÿ;?ì2üÊdö? ²hÐZÿ;4FGL J1303.1-4714¿îêaÑ4»ï@/,e@ÌxêÀ;$zØä2DÀ<×ïÖ½—@?$š"v?ü)tˆhî?ÓÅá @è(?çruÓÁ³"@l¨ýº«b?ôÿVø4Y¤?î¬âžž?àdÀÿß¿ÜGüN¿Õ,HÓ
¿í߯Þ)–|¿ïü2JÕç(UNASNone?ÍF¯~œ?ÆK™È~Àñ?è®y¼T Y?ÆK™È~Àñ?¦v|‡´x?»Eô%?˜7"¸?»Eô%?Ò^PVT}?¶zèÐóG?æÐ÷WÔÕÂ?¶zèÐóG?œ¿¹d× ?†}âÏê´9?ï*4ÙH?†}âÏê´94FGL J1304.6+0539¿åA—Pî5@QÂÀð À:çï¦ìhÀ<"®‹ÜB@£ÒW%V?þˆ×ªva?Շ-;!"$?àžÑç¾Á@}!"Î~@·ü—•³[¿ícƒ'ǁ¿¯^L€PJ¿Ûö î¿æ>$}㰔¿îxùæáK	¿ìšäó4?£UNASNone?ïJÅRÌ\?˜6åyZ¼°?–§U¼æth?˜6åyZ¼°?ïÛEÀÐZ3?‰ýÆBà•9?r]—Òæy?‰ýÆBà•9?ê}ª733?­™¦|æÇ?Æ	W#3Ç1?­™¦|æÇ?ìŽßÉá?¢'Þ‹WF?»‰·pø?¢'Þ‹WF4FGL J1306.3-6043¿ïþ6À{@ÊصýÀ8kÚÜZ	À;"KâC@•û¯
t2?ü瀭9Š?±=z	3?ÝXʜpäo@)ð$p!Ñ@ú F˜7¿Á"Ê|æZ'¿¬\w`o聿Â1ÅIö™$¿ÝM1a!.¿êŸwßµ‡·¿î»úýŒ³,UNASNone3FGL J1306.4-6043?gôäúj?c)˜èþ?ïèíè?c)˜èþ?Zõ´OK)Y?vâ*™¥‰ò?ïò…%ØZl?vâ*™¥‰ò?¥M"ìB?žY¯Ø¾^?î§ë.FÁ;?žY¯Ø¾_?
upHV%ã?<röÄ	Þ?ïÿ–*>Þ§?<röÄ	Þ4FGL J1308.7+0347?ígŸSY6@P'˜ÜÛ7ÊÀ:¤''%ߎÀ<1ìVu@t1ñê"?üÞ£©½Ô?Ð*¤CkºŽ?×ØJ"]?@_"YÒÚ@k‡ÞY[?îT  ô×®¿·]
½ô¿Ê˜\©#O¿ããBZ£‹¿ì™ V¸¿¼¸ÈúÃUNASNone3FGL J1309.0+0347?íÍs?ü?±}ž·Ë]?±—ügv ?±}ž·Ë]?ïŽ}m÷F/?¢wÀ}'÷?Œ`¤'.t?¢wÀ}'÷?辺qƒoÛ?°Ÿ‹g®)¥?Í9ò@"?°Ÿ‹g®)¥?ëËô‰ýŒ?¥áßяH_?ÀÐ/åØ	Ï?¥áßяH_4FGL J1308.9-5730¿ë7`;[V<@&ôàM/À:Ž 'F¿À<{æ*kä@—"§Šs?ÿü€ï~¨?Õ)ôzæ¦?Üxù!¶3@¨–2æ@¥¿p÷z? JAòh¾?ì¥~tz%`?Ö­Ò HÊÊ¿ãw?}ÄQ¿çæ!‡+¿ïÿž±0UNASNone3FGL J1308.7-5738?ë%ƒ"`Í?ÀjÂS0
ž?Ãióûv|Ï?ÀjÂS0
ž?îÏ©2cO?Âj‰DÍë?¯lÙË?Âj‰DÍë?蹃'n¢?³þ͵´"i?ÍóåöEx?³þ͵´"i?ê´.š¯¼Ã?ªåówæ›ê?Å/E•Aô?ªåówæ›ê4FGL J1309.1-6223¿ïÈU´-?Ùõ7d›5%À8âŽÕñÀ:é@oUxW€@ÃWEa3!?Àø:8àò?ÚzÁÈó@ÔÌ?ß ?öˆÇͱտïô;pïVe?ïì´É Èb¿âÀrM'À¿êÍ»à~í¿ë'jxÅ¿ïÿ÷Ò4ÛUNASNone2FGL J1309.6-6230c?Ó6ÒÄ­¯?Û?!Ç£¿g?æd–ò))?Û?!Ç£¿g?Á&¢¬6?šùÕF¿®e?ïÀ}²Äº§?šùÕF¿®f?£«ùŒÐý?¡$=§93?îÅ@g2ð0?¡$=§92?%Lš†ª£\?¦s'SZð?ïþ«6W•V?¦s'SZð4FGL J1309.3+8035¿ì÷ØOÅ@BALD|0ÓÀ;*qgKiÀ<xÓâjÃÃ@y7OË@ÖÕ"õÎ?À°àÝûÉ:¿º÷Tføˆ?ú.Æݟƒ?÷Od¤šS©¿ËÊõQÓ²¿â¥ôñ¯e¿ì˜¦ŠB䁿ćœDCÒ¿ë†lËÛ5E¿ïÿ••_xUNASNone?ï¿Ü`&³¼?'·â#kõ:?€çöS©?'·â#kõ9?í2æå?À>£š‡Cí?³~hÏOhÕ?À>£š‡Cí?îö‡8"4?–9€äA"À? —†üv¼Á?–9€äA"À?ìÆb
â†?ªúˆ½']â?¹ÏäïëÒ?ªúˆ½']â4FGL J1312.3-6257¿êÚ²@ǹ™¿ÇÍùóv"ÂÀ8š"O…yQÀ:YÔQüL@ (~oÈ@¡Tÿ5Õ¥?Á÷ZjÔÌ?Šƒç€­:@I=Ùb·@C›`C¿ícþ¬Bê?ï(SÜ '¿á"æ".¿æS®h]·k¿çqß
¼òd¿ïü"à՘MUNASNone?؝,>²ÍÉ?ÓëL_H·?ã±iঙ?ÓëL_H·?ٍ€¢Šu?×:afL?ã9?®÷ºÆ?×:afL?Þ^¯ÿÏ–?Â;Sl·™ÿ?àШqµ?Â;Sl·™ÿ?âp±}".?ÂÙ
Qr0Ô?۝üפ?ÂÙ
Qr0Ó4FGL J1312.6-6231c¿é´÷Uv²²?Ï!ٙŽÜÒÀ9QTsõ›"À:\Ä"Úœ@±öÃkO.@üØ:¿¯?Ґ`
à?Ü;\L‡@±žs.?üYçՑÂ`?åk¢E9Åô¿âŸ=ÙFX¿â1e"n"Þ¿âÓiÔ¯ð¿ë‰â!GÎK¿ì5?|í'UNASNone3FGL J1311.8-6230 ?£1K—"ò·?»ªÓ;šÀ'?îÌëFÐÕ?»ªÓ;šÀ'?ÄÆZa¨?Í"Ö)?êþig¿?Í"Ö)?ºŽ£ÛFá3?¨ÂQ:énn?ì®+"—#Ù?¨ÂQ:éno?°«û¾4{¿?šÇÀLÁ?íꀈ9pˆ?šÇÀLÁ4FGL J1315.9-6243¿á'g"Æ™?Œ¥šŒf]áÀ8rãËìÒýÀ9ãûó+g@Øçk´"@jZíŽ?ÃÌMß?;I§hå@ýœ¨?ãG_ºü?ämªþE띿§Ãހm<ˆ¿åwu³
"¿èœX@2õ÷¿ìPޓɡ¿æR£`—ÅYUNASNone1FGL J1315.0-6235c?ÂJÄÆ\?Ò½L_T?ëmzüh?Ò½L_T?¡úÔ!d1?¶è¨cWž?îàR½é¿ü?¶è¨cWž?²˜ú¼¼`d?¨t_M'n‰?í¬à¨hsô?¨t_M'nˆ?0˜É-ûl5?"¬ž|ÂCg?ïýìæÚ@'?"¬ž|ÂCg4FGL J1317.5-0153¿Û tn§¶‡@N&ìAÝ"À;DDfa]éÀ<ø0À'+ç@"¶'MÊä@Ôxã@¬˜?ÑùcCFPÇ?éizi~@}¯li¶?óQ½ØP:¿ïÿûÞ]Bü?ïÿØBKÔë¿ÐgbdÏ
¿é[O6Ÿ¿í"}¶98¿ïö¼?5õÛUNASNone?ª
Áø[g"?ºjY
‰J?î_SàzI‡?ºjY
‰J?®™z#'å?Á̈́…ÀÉü?îh]ÎwÒ?Á̈́…ÀÉü?Ə?[  ã?±õqÑ&Íy?ê\0)7×Ç?±õqÑ&Íy?Zð$Yý'?FvlëO¼s?ïò‡õmÓ?FvlëO¼s4FGL J1317.5-6316¿Û<JûÄ­¿áÄ* vmÀ8àÛÿo·HÀ;Ài;'@ÄØâ"Å@Ac?ÁÌm‰gÈ?â›êÂ+35@XÞô½²@Ì$'óÕ¿Ò¾0×@¿Ð¯ª}¬¿ËÈ©¼ýKñ¿æӉX=¿î<ƒß1i¿èPž¨øUNASNone3FGL J1317.6-6315?5(ã?Áw?*øZ²IÒl?ïý^šã˜?*øZ²IÒl?€i½¯þ
Ï?'}v`Ž?ï¾Y	@Õ?'}v`?…y»j_ab?jɍ‰ãÃ?ïªV'{?jɍ‰ãê?am	>¬È?J‰éyåŽ?ïî'öÁS7?J‰éyåŽ4FGL J1318.1-3937?éÕw÷vÍ@6óNÒöÀ:O!Kª"~À;ø>ü•u@¹:"úžA@¡{j×?ÀR‹vÁ¿ºº¢Óª?ô&Ã$º@ϊxis6¿è€zC'üÇ¿çC{[¿å­Á±ç¿éEP6y8Ñ¿ïþ3ý]ŽQ?ïöW_¸LbUNASNone?ïû3gðn?PWҖ	2/?C2`>Gã+?PWҖ	2*?ïӚmþƒº?˜´òp
?v2ɾ"e?˜´òpÿ?™gê?†ŠÀCçs+?ˆY¦;ÅZ?†ŠÀCçs*?ï඄"ÁÐ?c!"\m¼?oI{Ý>/þ?c!"\m¼4FGL J1318.3-1148?åÐ+›m6Ó@IBA¢a¿8À;8P©fÀ<þº…¢l@ °u±²ë?üÊØÞ¨—?ÌjØó!?¾úš ¹D@?õyç='@QŒõœNÖ?îåÑ0é­?ëEÅ.î*?´OÝà6r¿ç˜S~,Uɿ̙%•æ±¥¿Î•#éTqUNASNone?ïûÜ)
È?Eùs恅Ó?@ZÈß?Eùs恅Ê?ïûoÞÓu1?^Y$2¿ª?B@"²+<º?^Y$2¿«?ïÀ[6¾}#?€L)k‰hW?Òd ÁnÞ?€L)k‰hU?ïÇûˆ!»´?o<žãÀ?|;ï"%¬?o<žã¾4FGL J1318.5-6352¿Ø®™Ô4¿ò¸LH
À9ÿxǑúiÀ;
–}…fÝ@!1{{vn?ÿ܆铬ñ?Ò‡B)V?È'SV\ÿ?ñõ¿Ÿ½ 	?øVª0À'¿ês.0D?èRÔ¨ù¿êę!¥¿âŒ aßÄ¿à¢*aÓY¯¿ä²@¯rŸUNASNone?ëm	ßF?ÂHøLçFí?ÃÂKÛü'í?ÂHøLçFí?é e£gÄ?Ò«âM?É~ir`ïÍ?Ò«âM?ès²Cpq?³€ã"©?϶16ò>??³€ã"©?è…[BuÏ^?¸»{†ptö?Íê'ö(Š?¸»{†ptö4FGL J1318.9-4556?ïö*D+@0¨àP7PÀ:kÒPšLGÀ;ɯe³¹@ëÙá³8Ò@
•Ât"6?×n†›e!¿ æÏ#á~?×ÝلÁg@Õ(eú±?ï==B€®¿è;/`Àµ¿êD~d^¿âÔãâh'¿á,Ãã?l¿ïÿùµc#¼UNASNone?ïà蓟ñ³?rHàrD:v?ol`LÍ?rHàrD:x?ï(TïÌ°?´)P"‡£s?šõbŠ?´)P"‡£s?îˆ3ã?›ÐT;uƼ?§ŒÏÿñÈ?›ÐT;uÆ»?ï}Bë??{2¥[Úìè?W¢˜¿H?{2¥[Úìê4FGL J1320.3-6410c¿Í'wp¢¿÷£ÄzÀ:ћh¦³À;cp£×
=@V%üi@·—Ù¥ù#?ÒO/¾¹¸?ãšb‹»`@ãI{t¥@žtGP?¼¤Eoóe¿Ø®ÿÿdû¿ÝSV>PοèöуòÖ¿ïÿý¡UûŠ?ïçÚÄç%UNASNone,?Õz̔M‹'?Σ›fñJf?åB™µÙ:??Σ›fñJf?çsÝt ?Òî`7åy?ÑýE¿ö?Òî`7åy?ØE§™ñ?»é˜íL2?ãüÝ,3??»é˜íL2?äºø:H€ò?ºö'¼gŸ?֊‹nþ?ºö'¼gŸ4FGL J1321.1-6239?Ÿ&Î\ëz?oÒÃ(U¬À9F&yçL«À:=­P/Ã<@Cïò@Ï©@›çl‹C–?ÇmÍbôÁÞ?Ò7Ý ×ç@¼4 ˜ü¼?ÿ|ºñXw¿êö$Û?ﳨ~cÞ!¿äOÒ`_'5¿æ?_´Æq¿ì†väÝ¿ïÙ2ÁsR]UNASNone?¤2³œv¿Ë?½ùèf0Ëb?î¼ÔÆ8"?½ùèf0Ëb?¯ëûƒÏ?¼ä}¼J?îÎ@GÃ?¼ä}¼J?µ•÷ñâþ?£C6µëÓô?íMAAà?£C6µëÓó?¼‰mlXò?¬Ð® UýC?ìnÜÒRtá?¬Ð® UýC4FGL J1322.0-4624?ëoP¿7Om@0!y[5°¼À;¦v îÀ<ah#ÕÈ@õÃêûáã@ÿ$7í­?×Äzb?áƁŠY5@ÒõU'"@†Ùû3'¿ïö!Ÿ·ë¿¿èJ ˆK>?ïúÕÔ&]¿àwÍaGBµ¿èÝêa2Iÿ¿âG롤*UNASNone?ïI[ÊÊk4?š˜Wéè?–Ô†¦²™m?š˜Wéè?ïÖî!ðÅé?"û€Ïí
ˆ?tˆï£?"û€Ïí
ˆ?í´#þTV6?¡© uyeN?²^à
]NF?¡© uyeN?îbQu°#?˜îÉv™Rû?©Úè¤þ
Ã?˜îÉv™Rû4FGL J1325.3-5413?ïò³L¸6þ@ ž2~ØM4À9Д®xMïÀ;nS™Û@ŸOúi=0@¨˒:*?ÀQii¦î?Ð!û'©@ëÇ~¯2ˆ@1õ桊)?âìv Æ3«¿ÍMõVXÒ)¿ä=1NV¥(¿æ´äv]¿î^? ÿ¿h¿ïùÁ­UNASNone3FGL J1325.2-5411?Ê0Á³â)f?Á=ƒ"u?ésϓu¦?Á=ƒ"u?áBl@½?ÑHD€¼»~?Ý{é'ú…?ÑHD€¼»~?ӝé[Ë5?µÈÄÇLÇ÷?æ1Re|?µÈÄÇLÇ÷?ä
™8˜?±û9ßàƒ?×ëÔÍçŽÑ?±û9ßàƒ4FGL J1326.0+3507?éÊ`!f@SǘJAÀ:à=ûäÀ<Ð;êŠM@BúÑlð@¯_ü¿ÙŸ?ÄR†J1|z?À
W¬dM?ûL'"Ғß@!ü@­Å?ï4ãlK'µ?«5〇=»¿áËË]k¿á×>–¾ž¿ãúQjUß0¿ïýí5øàQUNASNone?ïüH¸¿jé??E%EÞO<?=º:¨¸É??E%EÞOd?ïüÄ*E!ª?QÒd ÕÚ?9Þ­Öò®Z?QÒd ÕÚ?ï٘ –?ucªt|?s3ï¿5?ucªt'?ïö&9ÐÄã?A3p`¾?S³Œ^v9B?A3p`´4FGL J1328.4-6231?辝€þo?§Ë@ےbÀ8ÎÍÐØËÀ:d3çüÔ@9´ú,V@ü``'çÏ?ÌŞÛô2?߃>ÄE@|h½X»ƒ?ô#Ãy<
?ï°iS?Ã~.Ú²¿ì!-Aª¿ëÕÕßðëæ¿ïu'Þ—$Ÿ¿ïÈzη3UNASNone? ÿ˜½ ñ?³z/±ÆC¹?îðt%ðî?³z/±ÆC¹?¾™CÁCb?Ê×ÅV¬Á?ì,םGד?Ê×ÅV¬Á?Ó¿$¬?·qև`Ñ?æ} wmö*?·qև`Ð?Tb_s?@¹œe<ÓT?ïõÎøwÐG?@¹œe<ÓT4FGL J1329.9-6108?îs‡;l?ö&Ks›ÙÀ9œ§ktÀ;^iŸÖÊ}@Ù؅½™©?ÿà,%!øx?½ø+஁?ÙÒüÇf[@710ýÏ@®€™B†¸?í½ÚÁ'ï¿Õ™0þz™Ï¿Ó¥!ÂÈg¿ã¿YG¿í-¢Ðzw¿è@<›'Á^UNASNone3FGL J1329.8-6109?dVo§ÂLœ?eXx­'¤¢?ï멐X=´?eXx­'¤¢?™ÐX{åÕË?¶ù b#.ê?ï1}< ÑR?¶ù b#.ê?2þ4	Èh?"Öl¿ä?ï~h_±¼?"Öl¿ä?Žt2~i.D?y07Eêx?ï†/6[G?y07Eêx4FGL J1331.3-3818¿ì˜ŠÛŠ€@7ç†
¢À;›í0ðcÀ<zÝ¢w@€?ÐOŽ3?ýç½f?àEw¾}~±?Ò€U$õƒ?õYžfý@µ/â›Á?ïœÒhî#¿é­è j¿â–-žž¼¿Î±£Ñ€ç¿ïhey×\s¿ë_oÒ UNASNone3FGL J1330.0-3818?ïõ
M€?V©ò:ð×c?UåÁdÿÒ¾?V©ò:ð×i?ïúG¯+"?g'y^³­H?FáC‡Qñ"?g'y^³­J?ï
 ‡íýÜ?"(Ï6áÉJ?žKï@Dr?"(Ï6áÉH?[Ù$+?t"׳eƒ?‡_©	¶õ,?t"׳eƒ4FGL J1334.1-4154¿íÊëu‡8@4@Ùè>B[À:`˜I7wÀ;ýːŒªž@¸0d÷¦j@é̂$2?À˜PƒÑl¿¬6ð/U?ç¡»Áâÿ@ɘ
²¿ïðG€^?îqu‹u•¿ë\dŸ¼ÉJ¿âj´>`ß¿ÙyÂ,_Ú¿æÒŸ½J#UNASNone3FGL J1334.3-4152?ïTÑ"Dà?šnG†Ÿ­?•eÜmwd?šnG†Ÿ­?ïå=Ó0š?•½é
h²?jÂ,Ïäfß?•½é
h³?î6gB¾°û?ŸOo¾æ?¬™‹ÔðL?ŸOo¾å?ﲕWÙE6?vÆÀïà?ƒZª	®²r?vÆÀïß4FGL J1334.6-4435¿ï÷ê,`g@1šP?³t6À:OÜ»WZÀ;þ†
˚ž@HÂÁ@lÇß'Bd?ÊWvßZn?ѤÃ,ºô?úßú Âî'?ùJ¡¶×¿á§úð̆V¿ç­czù›b¿ßí´ctn'¿ípÜá¿ÝwGʙ즿Ð}U–4ŠKUNASNone?ëÅõÌP*?¿&¬Sã9;?Àè(οUÉ?¿&¬Sã9;?ë‡è¹æ¡»?È51rÛ6b?Áà]ey?È51rÛ6b?æ"cBoX?·7Õ,51?Ò÷9{!P?·7Õ,50?ëÆêÅö?°kˆ°½?ÃÜäWìè.?°kˆ°½4FGL J1334.8-3856¿Þ«ßÞzR@@7("Æ£½àÀ:TqËõ6xÀ;í½îãx
@^¬ÛA@0!ùO×?ÁÀâ]Ø£¿¼jØE²?û­N'D?ú/}F'?ïôòñ#Ä*¿é-€¡{k¿äºïÀÛå¿æRuþ´ÑX¿ïöö¡²lÏ?î3Œ>½*UNASNone?úö°1?£‰å"g…â?Ž"BSó‰?£‰å"g…â?éjG,pú)?ÎoL;4ñ&?ÊVãN<]?ÎoL;4ñ&?í­Þ¸?¨æ}w,W]?·Ïâ'òA?¨æ}w,W]?묽o$ov?²:ƒqGm?ÁM
CnB)?²:ƒqGm4FGL J1335.5-4546¿ïÛ·…/@0ií9SÞ¤À:Ao.ŒÀ;û~ÿº_ã@÷ `ȗ´@ßݵR?ÈEF³î…?ч¾û¨ØQ@5]¢r†/@ÔPXÝè?äčc*qÄ¿ÖÛh›õ¿_¿å"øD÷¿æ"6 M}a¿ë½ËrY¹°¿ðUNASNone?Ü°jèÖë??ÆÂ~=®Á?á§Ê‹"Š`?ÆÂ~=®Á?àm»Šõ-O?Ñ;"žãžä?ß$ˆê¥c?Ñ;"žãžä?Ý;lÅýª?¹é{ôN—?ábIq+?¹é{ôN—?àgÌÁãÞ?±«™ê"Öf?ß0f|8CÍ?±«™ê"Öf4FGL J1335.6-4052¿ä¡Ÿ:Üîü@5;n.±Ä3À;^bMÒòÀ<…ú¯^&ý@!ì¿	ª@Óª6ŸÏ?Æz}ʆ –¿ÁÚèÄO%?õ-§¾Šà@ƒçÚ«?ïø˜,²²¿ìCË0ëZ¿ÚÌù"@F¿ï/<=Èã^?æÐ;·f3;¿¡Aµ)ßUNASNone3FGL J1335.2-4056?ïÿ^}?$î¬kÀ-²?t0NNk›?$î¬kÀ-Ì?ïüO´º?[
š±L¤?=‡šZ/÷Ý?[
š±L?ïÏËý7Ã?~õÀ?xäË?~õ½?ïúGc¾?HRa¨"?Fâs¹Ì"?HRa¨34FGL J1336.5-4655¿ï¼iûëÞ×@.}â:óÀ:Akn
#ÕÀ;úž#lÓ@?£v'-•@éZD4"?ËZX¦ŠBå?Î[Ähû?ÿÓ8§z¢@ú…"áQ?Í&ý…Qc¿ä,È`›±¿éšãEµ¿äAÃ^¹ô®¿îq‹'æÎ×?È}+å6%+UNASNone?ät¬ò5\?Èû¡!û}?קè•H?Èû¡!û}?딳¯ü™f?ÇЪã&x?Á­1@
ši?ÇЪã&y?å*<Õj™?¼{`•=(q?Õ«†UÑ*Ð?¼{`•=(q?íÈeËÇ? ±Ï
#`%?·Ù¿dÑ¡Ñ? ±Ï
#`%4FGL J1338.0-4159¿Üîtf@4
šÃeDþÀ;
ÔoX}À<‡µ¡7Í@  ÍâK ?ú²?'ÌÎz?ÕòÄMã
?Ò¥kŸ`X@(‡€'a—@Ç°-YÕ¿ïöÊÍL'?횣"Ôæw?֓åDè½C¿ß5î#‰œ÷¿ÍK€†ù¿éÒ%œq».UNASNone?ïýˆ…Í?6¯Ä`EK?3÷C»Ñ˜¼?6¯Ä`EKª?ïûšÕêó?XÛè©Îö³?A"¨T3ö?XÛè©Îö²?ï±÷Š6<?'xÎ?‹'i?ƒ¹rpÞ?'xÎ?‹'l?ïø4ró¶}?@{#6«Ñ?O.41&
r?@{#6«Ðþ4FGL J1338.8-4509¿éóÂ"Áåx@0çm"BJ'À:·)Æ¢ç À<6,ém"@MCtôɖ@ËHûòTF?Âü¼Z
è?pý
~Êeˆ?²y=®ŒDò?øà‹ÓÞ9?̙ŽŒ"Ž?éêô€­¿ç

Ÿû³j¿å¨šÞ"Ô¿æ60ÞÅÕ¿µ8äx0JUNASNone?ïvØ]£È??ŽºCnÍ?'$ôK†ø
?ŽºCnÍ?ï154'Ò?°
Å÷Â?™ÙYo¥¿(?°
Å÷Â?ïpMn¹Ñ?v£ÎÊ?'ö\'(Åþ?v£ÎÇ?î$Z±r+Ä?—ôèZ?­ºTèÝCÅ?—ôèZ4FGL J1343.5-6827?dµËÀHŒ°/À:ËCæÝõÀ<,Mâ"s@=;"@óÅ¢6 M?×*Ÿ[$"Þ?îÍ~d^N@f"»ë@;(ðÁ?íÛûß	s¿ÖAcAî·Ù¿ä(³GÀˆò¿ï춬Ï×C¿Æ¹Ä1r¿¿ïá½õ™t±UNASNone?ç v»ÌÛ³?Ë¥&VM–?пˆfHš?Ë¥&VM–?à'ðwº?՝·VZ(?ÞÛÀà‹?՝·VZ(?ٛ=O«
?¼ˆŠF'Œ?ã2aX8*{?¼ˆŠF'Œ?ÐT³XD?ÂüíPcCî?çÕ¦Sñý^?ÂüíPcCî4FGL J1345.9-2612¿êŠ-Z(-"@A‰:'£SÀ:¹Y×êðÀ=£.mѕ@©t$j¡@Ç<t$•?ȋË:PˆÚ?ïþƒ~$H4@&\âY&@	>èŸf7B?íPŠ\õ¿ÚrÃ×ZÅH¿©–Ú]À5Ì¿él«úÅ-œ¿ïÿþøþ"?ïj8$óTUNASNone3FGL J1346.2-2608?À5ޏxÅ?Ȅp¬C}¡?ëý2ˆ\!Ï?Ȅp¬C}¡?¼m¦™\žž?Ï~ˆ*yG?ìrK,Ôl-?Ï~ˆ*yH?Ê
ßèo½?²—²¿#ë@?é|ˆ<Eä?²—²¿#ë@?žýâ:Àø?"ló
=l?ïPî)ø?"ló
=l4FGL J1346.5+5330?рUx
¸@NÜz¿¹¾ÓÀ:h™î˜ÏÀ<ž))Äõh@œ³ì+6å@ö"ï¾i?½–Öñ"×?¹6w‹QØ:?÷W›ÈH@§¡§…§?êà^úâ4¿æËÔHµ{¿é€NÚX¦Š¿ç!ßeUÅ¿ïù¼º0¿Ù&ðކßUNASNone?ïÝV!Z7‡?sË`ðøh?qTïRä<f?sË`ðøh?ïR2Žgî]?¤­Á€V?•¹®34b?¤­Á€V?ï¥×öy{?ƒqyn'!!?†¼Ja¡?ƒqyn'!!?í¯
xy«? Ï̎'Š€?²‡ç¬<2ª? Ï̎'Š€4FGL J1348.5-8700¿áh«i‹oÀ8;*'ñ¶'À:ˆ cLÖrÀ<2
˜à66@ô%8Kv@Ô¼÷"?ì˜ôX,¿½­‰:¦Äû?Þd¸[¦™Ý@	D&{Ÿ^?Ñ''?X¿ãáÚ{9¿í^lœáL·¿ïþÂþ—Ë
?ïñhÃ7ø•¿ïÿ'ö֌UNASNone?ïÿ¡Õƒ¬?y[W10«?ŠŸŸú?y[W10ë?ïý‡6Â^?sQ÷ßuÜó?3ÆIí!;?sQ÷ßuÜò?î÷êOD? mèö-¬F?£ÏD[È? mèö-¬E?ïÿËB X?ËR[6Qû>ú^¯ÔR?ËR[6R64FGL J1349.1-5829¿ê'Ä5‡ð@Rºû15À9'ðrÄB»À;TkJѵ@ÇÏÿZã@ù†üÞãP?ÇSÖö·W?½0Ãj¥?ö"fÿéYË?ûr—w*ƒâ?ïÿûÎBÓ¿àxŽ¡îÒ±¿éñ×HPѪ¿éނö ¿Þòb+‰ò¿ïš¢ãÅ6ÖUNASNone3FGL J1348.5-5833?ï¸<i2?"~ֆE=?þðû%³h?"~ֆE<?å*™»ë?Òk[£a.¢?Õ«Ê̈)ú?Òk[£a.¢?ì•x\Ãy×?¦3àÞ 7N?»T=ä1G?¦3àÞ 7N?çiÂ?Ö?¶f.YÁÌÌ?ÑÕ,{ӀT?¶f.YÁÌÌ4FGL J1350.9-2757¿Í÷[¸£üü@@ŒÜY1ÊÀ:z(4Òo¤À<Ç]!CG@ÌÆHy@‰@¢\›âI6?Í{±ýºÃ?Ðé̂$2@;#Â|è?þ9—ÒÅ¿îðŠ!«¢?ïDŠ=Ü¡¿ç®ùþY¿á)-÷¿îk½Þrf¥¿ïìœ
!¼UNASNone3FGL J1351.1-2743?à¨R«°Õ?Ël"¿\‹h?Þ¯Z©ðžW?Ël"¿\‹h?æ¬{л­'?ÑòØ°Ld?Ò§^ˆ¤Ú?ÑòØ°Lc?ᵨŠuÉ?¸ùš	;­|?ܔ®ëÞn?¸ùš	;­|?Û÷!ÉDú?»†J|??â|"o]ƒ?»†J|?4FGL J1351.6-6142¿àԆ°y'?ÕÃí_êKcÀ7þ§vÑîuÀ9òzƒSÜ÷@Î$ªYZ@(H¾µ²Õ?¶>$'ýu?Ñا¡o%þ@ƒ(ùôMD@n,"Þsé?ì›Æ/#Ùú¿¯¦^B¼¤¿äÛé B*G¿èõ~ò¤M¿í3nŒ¥•P¿ïÿúVrÓ\UNASNone?ÑmžO*[¼?ۂf]ì˜?çI0ØjÒ"?ۂf]ì˜?vd,Ygi«?r±åìu?ïÓ7§M1-?r±åìu?"ü!j÷=?‰"Lß!=?ï`÷ĨF?‰"Lß!=?FãmÄ?8ɧÕ8®Ö?ïúG$¾¸{?8ɧÕ8®Ö4FGL J1353.5-6128¿çˆrM­J?à´¬Ã˜À9­ê‰v6À:DmŒËU@ !€
+Œ¡@Ù\T"­?ÑÜ©ò­1?Ð¥·_'WÞ@–ѵ(k@_ƒmÞ)ì?ïQ½ei¿Ù¬bÉù³¶¿æÍØÀË◿稊-¿ìèÜy¿ès¥J_ UNASNone?Ñï}Ï¥/u?γÜÁÓ?çA-hF?γÜÁÓ?Í.ʈÁÇÌ?Ðø¸_		?è´M]ώ?Ðø¸_		?Ò½sbmL?¶VL0µ;Œ?æ¡FNøÉZ?¶VL0µ;?È ŸdîE?²îþ½òf?é÷Ø&Än¸?²îþ½òf4FGL J1354.2+0353?çvr|Né@O,*^x[[À;]ôiÉÈ6À<®$´ë.¸@ ͇‹z&?ÿÄXŠÑ?È[XjËP¿†¥VøE‡°?ÀÎ2èà~°@9ÂÌÓ?ïðp
TÙ¿æo^݆Ž¿âWʌ€¬c¿ìI!ñ¿Ë?ÔÉÛÁ‡I¿Á•ãšzUNASNone?ïý–_?>käö·n?7K}÷?>käö·i?ïýž•V¸ª?JV Ëî{×?3UJ:°?JV Ëî{á?ïÆ8$%ö?€À'Ђ§?|ãííþ~?€À'Ђ¥?ïù?"¢0ê?Eß6Àé™?K±w<T¢?Eß6Àé˜4FGL J1356.0-6747?Û«PL¼bÀÄSK×nçÀ:RebZh+À;Â)©FµÇ@¦¿Ë1—'@¼¬ùÈ®Z?Óˬ¦¼—Ë?è-3¿Ë¤@yl$ìH"?û[9i®ƒ?ïFòbˆ‹T¿Ý½<‹÷p¿ëXd"¿íÁED­®ú¿ï¼~Æ.£¿é—€ŸÍAUNASNone?ÙRÜb£G?ϑÕb't?ãvV'ή]?ϑÕb't?ٛ‰¦
†Ï?Õ¿þ¡ M?ã2;,ú¼™?Õ¿þ¡ M?Û%7ÑþI9?¸bÒrMˆÐ?âmdÛb?¸bÒrMˆÐ?¢iÕgÓ{?‹Ê¡ÅÏmÄ?î×éb©'É?‹Ê¡ÅÏmÄ4FGL J1356.6+0234?Û4+^X9@Nt*€JÀ;ÂÀð À<Úü›ÇqC@úk­ø÷"@ë=Ñ?ÐmÝvV?éºÅ˜ûäè@ô]…TÖ@ûlYA:¿åÝlÇ©w¿Û É8Õì¿Ç8ÖöœT	¿éŸxÁ1ãþ¿ïÿÿ" 5•?îƒÁ@&¶£UNASNone?×ÚNÁ˜ ³?Ïà'72°Ì?ä؟3¯§?Ïà'72°Í?ևËON}?Ô­RJ`?ä¼pšXXÃ?Ô­RJ`?ËÖ{
Ý~?µ¢åïgÈ×?é9Ja=H¡?µ¢åïgÈ×?ÚÂú°ë{?¿ItŒ*`ž?➂§ŠpÃ?¿ItŒ*`ž4FGL J1357.3-6123¿î»¯Àœ€î?ސpõ³ À8ïåÍNÓÀ:æ	´´¨@7‰Ia@ŠR¹á7¾?ËÛ)†âñ?ß[_!M­ˆ@þª°BR‹?ÿžwì©·¿á$rÀç¼<¿¨}ô]ƕâ¿ÖÝË!Ñáà¿ë·†Ÿ@øn¿îÿãIœV¿èD?JÑUNASNone?†°±èçÀs?Âf|øw?ï¥=8\`þ?Âf|øv?©ïåbڇ ?½8"¦Ú0C?îa©ÒW…?½8"¦Ú0C?¢N&¹¬Ù?Dã [~!?îÞë"e3?Dã [~ ?‡ù!Ý%®¦?uå:|£?ï x‹iF?uå:|£4FGL J1357.9-4907?ït¯ÿ¼›y@(¡™V}»À:ÜþÒ—À<¨Ï—'h@¬Æã#@¿Åäë?ÅÓ\ÉY¥¹¿ >ªhR?݊´cõGë@z²ái<?ïÿ< A¿¿æ…¢×/ý¿ì·¬ª–¿µM`:—¿è*øÒU-¿Þû¶YÃÀµUNASNone?ïò€;ÍÕ?cßÜnq£»?[èÿˆdVº?cßÜnq£¿?ïÕÕ¿î^?šÆ~¶LÍ?us Ñ?šÆ~¶LÍ?ï_Yšäu?-ZgRÉ?"̯Ãqm?-ZgRÈ?ïÚˆÙ¦?b±JC?rô;ñ",þ?b±JC4FGL J1358.0-7749?Ì	°8kW]À.Ök\šÀ:{@¶©tÙÀ<)ŸY@J›÷lÞ{@̳_=}9?Ìu´øo½Ó?Ç{V¢ùê'?üû=ÈK^?ø))ò—·—¿ÄÏ8
û¿âs~&÷f¿ç©>RK&¿åãHÿù¿çú¢'ݔ›¿ïÿ/‹_UNASNone?îðŠY\?¦é07`;•?¨€÷ZjE?¦é07`;•?îP«vRëõ?´iøRR
Ÿ?ªõHšÑ@²?´iøRR
Ÿ?ìyC¿¾b?®GA@?¼5âð?®GAA?é'X_n?¨¾@§Æo*?ɺŸ³þ'L?¨¾@§Æo*4FGL J1358.3-6026¿ïã6¯yg…?õƖ^¤ÑÀ8"n°'-À:d>XˆW@x=û»ù@‰¤Y=?±XR&"g¦?ÑyYˆ1'@@@&`½?ÿF
ñ/W±?îöø_LÁ¥¿Óîtý­ë5¿ãKíÿ¢b¿èÉf@¿ëÓß ¹ôX¿é3€`°UNASNone3FGL J1358.5-6025?aM ¾S›é?ŸïmM1Á¥?ïî²_A¬d?ŸïmM1Á¥?z²IHúo?ˆ}åDˆÝ ?ïʛmn?ˆ}åDˆÝ ?Šd§ë¸<V?€
ƒkŽÛ?ï–m`Q?€
ƒkŽØ?E;Õ~†§?4Í£übB?ïú±
 ^V?4Í£übA4FGL J1359.5-6615¿Ñ;9¬IPÀ&0"ÝzšÀ:wŒ 4RîÀ;¤»5˔@Hàø'ï]@yYE³Æ?ÆÅÒG5Ä¿¼·^""m?¸ßw^Ü.j@ú\­U
N?ïôÊ(,o¿æР@ý¡+¿æ'³áÄU°¿æWæ`ǖ¿ËTO£uœ¿ï¤œ—zÛhUNASNone?ïڛŽä7?kêY/S³/?r²8±
äÅ?kêY/S³2?ïü»I{A`?b2h@ÀW?:%´%õ?b2h@ÀW?ïÈçq?"
NRjü?Ÿ?&ãå?"
NRjû?ïÓßî?e–S
Ì?vrðr	¡?e–S
Ì4FGL J1359.9+3616?îÖRq]@R5!…Æ~À:¦ªWVþêÀ<"웟-W@+èJ%@§†
¢?ÃٚæuÀL?¬jÐa	Ñ?â%ëoOC@"N0"Þ¿â¹_'F–½¿ã¨"ÿÔò¿êÀÚPC¿ïØ]ÂRö¿î媞ú'¿Ü¿³O÷9UNASNone?ïø…Ê©äP?S£Ïò؅?MèÕXnÁü?S£Ïò؂?ïƒæpçy?¦T€³NRa?cøÆ!´?¦T€³NRa?F¿¶÷?‡z ÂØ<?^.PBA?‡z ÂØ<?îð/eËب?'ÃÅmUd¦? ý	£Bu…?'ÃÅmUd¦4FGL J1400.0-2415¿ÕQÌ•Â@Bt§qÉqÀ:B¿ö$´ëÀ<}+é'Ö1@%Ù}_QI?ûÎ:Ufcâ?ÃÝýâŽl?ß(Cëè@fX`f@ŒÀ0Ýž?\X¿Ô¡—Zû¿Æ.·ùVº¿ã[ãU¥N¿í€<›'Á^¿ïË!6±mUNASNone3FGL J1400.2-2413?}'峃³R?z²¬q5?ïÄú4˜øš?z²¬q5?ŸÊHò'?¡ÚzÒéµ?ï¯M¿ o?¡ÚzÒéµ?"K—Qî¥l?ƒJ°»`ъ?ïe£EpŠÕ?ƒJ°»`я?§ì'%€Fh?Ü•-ÿ|{?î6í§ûš?Ü•-ÿ|{4FGL J1400.4-6050¿ï2IáY?ìóŔÊ'À9·ÓôzùÀ;CÓÀí@l§"W`9@΍F¤ÿÿ?Ѷùü°À'?æ†\㔏@wàmò@ÜòJµ°Ñ¿å>, òÔH¿æ¨!â}ä¿Ñ}Ýï<¿å.	"&¸Ñ¿ïÿý`éNä¿à–
~C›UNASNone?Ë&$~Õ¥?Ç:†r2?é6vàJ–¹?Ç:†r1?Ï3ûœæÕ?Òà¦ùï"?è3;ÆJ?Òà¦ùï"?ÎîŒþ'ÇF?¶ƒõƬÊÄ?èD\À_N.?¶ƒõƬÊÄ?ÕD'=ê9f?¸ ¼öQ¹á?å]¶á
ãM?¸ ¼öQ¹á4FGL J1401.2-6116¿ïZÀE-þ?ÞQ%ʟÀ9[(5©/9À:Ób¢Œ‡b@·:ööìÜ@ª`üšò?ʗð!:¸8?Ù¿E» '@
	_à:gÛ?övàœià¿íD]Ä×5?¾æ]Â}ée¿Õ˃ÁÁ¿âÎòJ¶Ý¿ïDá±``?£Œ'ìG-UNASNone?í¯DA©?¡•.]eGâ?ïȒ…Ýô?¡•.]eGâ?¨.¾þMR?¸
#.w6?î}4+?¸
#.w5?¹ü¯c÷}?§Yµ0¾y?ìÀjÑ?§Yµ0¾y?˜ËX_E6b?†~ eÌðX?ï9¥=ÖM?†~ eÌðX4FGL J1401.3-5012?ïëO¿®Æ@&Aòý¸ýãÀ:SQ÷GËÀ;åF­czú@1ʨZR@vÜB‹•Ë?ÉŸY¢Ò?ÃsÇ¢ìS¦?öO²$ªÚ4@›±vÚþ¿â¡{_ò®ß?ïõ–Ÿê³¿æ¿a>ß8à¿ä¾É¿Q9.¿ì¥Xtá¿ðUNASNone?î—þEbc?¨€ï!;´1?¦€©ÙÏ#?¨€ï!;´1?ëó>¾»Q£?Ǐõo7щ?À3¹u?Ǐõo7ъ?ë9ÚìŽØ³?­!ú0ÏÌe?Ã"Mĝ1?­!ú0ÏÌf?ë÷lScñB?ª=æWf?À"N²p:ö?ª=æWf4FGL J1401.6-4645?ÝÑt ¯á˜@,×`Ï‰@À:_!©ó›À<Á±æ—y@×\Q9®w@æ¤ì´?½x؃å'b¿±=Þ^p?ó{;	ÁIâ@·•‡U
¿¥ò¨ êé¿é
á,ˆ¿é//˜sÿ¬¿àC݊¿ë$®ÖAÀ•¿¦&™áÔpUNASNone?ï£+œQ?ƒª=>^"?‡5Xë¿5?ƒª=>^"?ïæ "£Yœ?‹Þ–ó€"??ißl\¦d?‹Þ–ó€"??ïrH16Y
?ŽÖ¢Ÿ(Á?'¶ùÙ4Þ²?ŽÖ¢Ÿ(Á?ïÐÀ¢y?cµþ¢ä'?wŸÿ®ÃzR?cµþ¢ä'4FGL J1401.7-3217?ét§L7A@<EB€®IÀ:½–V;À<x¸Œ£è@WrÜÁb?ýTyð'Î?Õó!à¥q¿?ÖÂhż7S?û\ߺZç@QG9Oó?ïyn‡P¿çl…>õ!¿âãÊ|"¿ØŠYàœ'¿è¬¦Q8ø¿ìžÑÿUNASNone?ïú9ké'
?K<D<R8?GPY»×=?K<D<R8'?ïý§2ïP?KŸGšs|?2Æh…'Í?KŸGšs|?ï{ÀGè¶?ŒéN×9¾?‡÷üé=?ŒéN×9¾?ïꠕµæƒ?Qª>Ìó?e_jJ|9?Qª>Ìô4FGL J1403.5-6236¿ïØEå=¿ìD¤¿èbÕÀ9NûH
[À;ži9}@ŠÊ"£n@í÷­K'?ņIÖ©?ï›ü€¿@Žï¬.@ËÔ²IhÕ¿ïÿÝ/ñ_S?ïÿp\‰¿Â©•e,¿ã¼ì™.:¿ïÄaùð†?½•æܘqÑUNASNone?b)Ä@Ó?¼Ùv^ü¨/?ï|î±Ýûò?¼Ùv^ü¨/?ü~ð¥?"]˜Ñ"p?︯°=?"]˜Ñ"o?³š0ú?¢º˜‰X:?í¹ýÁ?¢º˜‰X:?SFн91U?C3ãRÔIZ?ïö\—¡cf?C3ãRÔIZ4FGL J1403.7+1513?Ñê#¨#•@QZ0#̎À;hÙQ?µÀ< cÞÌ©'@A_ˆhš@–•3®?ÌOÈ?—Á"¤+1Ì?̒ ¾ç[ï?üŠQՃ¿ïÿÿ" 5•?ïÿúVrÓ\¿ç' ¤:\¿ãUGá‰ó¿Í–õåÊʔ¿ïÿ%¿Ø·UNASNone?ïøñ­$Ú?P©¥R£¨?O´9Kl˜²?P©¥R£¤?ïôÙâÝ®?zם<ÅÐn?WîL:D¢Ó?zם<ÅÐo?ï´âš0q?€°jŒÐÌ?'ÇYsû#º?€°jŒÐË?ï©Eý4,Ë?xšªÅ¢í±?…®€²ôÍN?xšªÅ¢í²4FGL J1404.8-5237?ïáçOàÓN@!M¤¬ó²À:lÚ"À;癴qŒ4@NMlDvÒ@ˆ¢ù"«ô?Á6F8¨²?Е§œ'›ž@	ŸNÒö@+Å ¿Ë,a‡ÚTu¿ç¼"pdìê¿Ôïʓ6©	¿æÖÜH¿êþz#²Œ°¿ðUNASNone3FGL J1404.3-5241?ßôû¥ª?˂6TD%¯?à'-|7«?˂6TD%¯?áݗ-Kó^?Ò
£>GÆä?ÜDÑ¥hD?Ò
£>GÆä?Øbr]òû?·]ú?ãÎÆøQ'?·]ú?äv¯)?²]ªäüf?×С٬þ?²]ªäüg4FGL J1405.1-6119¿é¡Ñdüc?Ò&Ÿ;š
À7€®I#À9iÞÎW@	¿Bu›c@PŠ"Ràx?±M
NóA?Ñ(6À[zO@"µz»ˆ?öŒ¯˜ß_w?·Ë¼V‡÷¿×ˆï]J¿æ«"zuè¿éç.þL²¿ë'®/RÓâ¿åï@4£UNASNone3FGL J1405.4-6119?p[OĀËr?¨;-2?ïßI`vþi?¨;-2?_™<+$YÏ?jcµݓ?ïð3aêmÓ?jcµݓ?¦imf߂H?Ÿ›»[×3å?î™i)'Û?Ÿ›»[×3ä>Ù»Yõ\ Å>ÓUC-QE?ïÿó"SR>ÓUC-QD4FGL J1405.3-6008¿áoóÛ9\?ö«#/¯ñÀ:4äR´ÙÀ;^¤€}há@!¹ÙNehº?ÿ7½¯lj?ϧWGd˜†?³TÐùøT?åóÕº²@ò^ªuÛ?ì‹m¡Ä
†¿ënÁê»m¿æìma,j¿å!Á›Á<¿ÜˆC{)ìã¿ß]©~i'UNASNone?ïøñô"›Î?Qšô˜€Ã?L8/uÆ!?Qšô˜€Ã?ïâϕ¤-?že™ú>^?m0jo[Ò?že™ú>]?îëý
>'Ý?šû5Mg)Í?¡@/,Ò/?šû5Mg)Í?ïÊýém8?p¯ÙÖSŽ0?z÷Icä?p¯ÙÖSŽ/4FGL J1405.9-1853?íêrÂX@DHFà!qÀ;!¦Mà^À<\m¿ <@ Ťö!d?ü;cž5	Í?Ô-ÁÚ*ƒ?Å(ŒDâ?ì%Õ²NœE@êŒÒ‹Óˆ¿â*"Q€ü¿í#¸Œíº¿À'\HÖ2§¿çKýî,￟‹råOпïÿþÞ÷UNASNone?ïÿ:QŠC?q…"tÜñ?µÎ¿ÂX?q…"tÜà?ïþØŠñ?G?]ê1×?/~÷PóU?G?]ê1Ç?ïÊ"
ÜÆé?|&~j'ÃÂ?zîú'œ‹Q?|&~j'ÃÀ?ïú;‰T8Ø?=LØ~ß!?GÚ¯ Æ?=LØ~ß4FGL J1406.2-7500?ïïÚ¬<À)²<êlÀ:§‰i ­ŠÀ<ÖüÑwV@Ðҕäƒ@¾6œt?m?ÈG<)¦íj?¢'­€™l?×VŽ®˜.?ûµ¯¬ÖbM?êŠÍÿ&ç ¿ééH-–;¿àHe)O"£¿ë›—jë0e¿â!iÂ;yS¿ïÿôa¼2¡UNASNone?ï÷'üh,è?Y"C°çª?PÜ/¦0?Y"C°ç©?ï—D »?ž)ׅ(Y?Š.ÿ×øö?ž)ׅ(Y?îùª8C'?•(™SIöÞ? nõ\{͒?•(™SIöÝ?ï;R¬™"¾?"Ñ™y$??˜•ªlÏhR?"Ñ™y$@4FGL J1407.4-0820?ïù]Æ6@IÄ"`À:¹Š '§À;¶@­o9t@¦óˆs@W£TY?ÌYAºµs¿£ö傮Ï?̎EèíiÐ?ý 'ç´¿ÔîYyîÙg¿æÄe©¿á€C‡>MC¿î*Ò§a)? ^vÔሿãHû"±UNASNone?ïõ€#xq?a¨Õt
êÑ?Tÿ¹ò'?a¨Õt
êÒ?ï㒲Éíä?ˆaêbT?lmM6‡?ˆaêbS?îGº†KUO?›Ùwgы?«"W›J«
?›Ùwgы?ïѕô
à©?o£)RW€ª?w5ú«R?o£)RW€ª4FGL J1407.7-3017?»°ª:Ê@=ÂNY)gÀ:Á°\S½íÀ<"(LOcë@¾t@ꗃ>äA?Îþhö¹…?ë©hyfk@W[_¢'@ûr'¦
?ÅRHw=#L¿Ó?š_<P"¿ãT5â:\¿ïhD¿ïÿÝƒ(i?îœtÀFV¦UNASNone?Ý	Ý`:r?џköøZ'?á{OâÆþ?џköøZ&?½lÃý¤&?Æ|Fí¯è?ìRg€K{=?Æ|Fí¯è?ÓdŒ¾Ð£"?²¢h'Ž`<?æM¹ —®o?²¢h'Ž`;?Áï*–¨~t?°Ê߆¬?ë"5ZUàc?°Ê߆¬4FGL J1408.0+3834¿Þ´©çå@Q"-¶°`À;·¦ a4À=d2‹n@ ²->>T?ü̳¢Y[¼?ӚµUů?¾àŨ]_?î¤âè7Œ?ÿûR[Âsƒ¿ïږ";cƒ?ïõ·!iÝ¿çè§ô¦/ª¿Þ¯¦/OÏ?—øpƒd'À¿ïÿÒ³–šâUNASNone?ïüžèÛÁ?@h4u‰hÇ?;¹!÷3w?@h4u‰hÁ?ïûÍàˆÛ?XB9ƒ /?@˔}ܖÚ?XB9ƒ 2?ïÖPíTm?t »gקÀ?t׉rÕÉ}?t »gקº?ïؙI£"%?iÓ _/?s³[.5í|?iÓ _,4FGL J1408.1-6010¿ÏÿfÍp?ô¾C·å´ûÀ9¹™	PášÀ:écyL8@ o+ˆÄà@õþÚf"?Ðli_À?¾"PTVC"?ò^FtŽ@–‰nÔ¿ïùJ¿@ó?îÄgÙ--`?Þ"ZÞGô`¿Þ8_~¿ïû ŠN¢û?ï˜l]vRÃUNASNone?ìówYJ	®?ºÞèúžM?¸dE5¯²‹?ºÞèúžM?é(¼­?Ó¼иå ?Ë_©½
½L?Ó¼иå ?çà}ž7_?³ÔSžÀ?Ð?ÑAö?³ÔSžÁ?ëÚñQ:%?³!,0ǤÅ?À";æ»j?³!,0ǤÅ4FGL J1408.6-2917¿ÞWÑÃ`Ü*@> í_‹ÎÀ9¯»åüjÀ< ¬Ö(–@$ë,ß1@æ'öÀ?¶õIB¿X?¶[âÿ¿z?÷`ýV"U@]Î_ª¿ÐUýfȌ¿ævA:\ó ¿éÅ(~#qt¿ëp(¡ß¹9¿ã²€áü}¿ïí'ûî£UNASNone3FGL J1408.0-2924?ï×´V¦Z?sؔl
Z'?t%ÀT¬Ò©?sؔl
Z'?ï÷NªÂ{?±NªµöIp?Ÿ!*§°–?±NªµöIp?°?™-èW?§Î÷î+?™-èW?ížÓÛ(l?¢#‹'ÜŸ?³	a'æ¼¢?¢#‹'ÜŸ4FGL J1408.7-3747?߃}{nPÆ@6™Å£ãŸwÀ:˜³"&jÎÀ<`% Jù#@M"òiG@Os²Lï?Êz:°€?ÙqR=9œY@Wކ2´ˆ@$ð"ê¿ïÿû-2h2?ïÿÚÁ,/´¿Ý¢¿³Öh¿åø!ˆ¬6¿ð?ïý¡ñ&UNASNone3FGL J1409.2-3743?åâÝ£?Êì,²[É®?Ô:D¹ÃÉÄ?Êì,²[É®?à˜)‰êa?Ô®ÇÜÎN?ÞϬzì+=?Ô®ÇÜÎN?Õ[-ƒ4åq?ºE×ÇVÓù?åRi>eH?ºE×ÇVÓù?åAÝr%؆?»Ù¥Ñ9¸?Õ|E´Nö?»Ù¥Ñ9¸4FGL J1408.9-5845c?ÐàÛ·íØ@õöº «À9#¹À;íöé@Ê«V™m@Ìhĸ*?Í.rýMž?¬ÛMîöBg?ä£þwiÄ@$ˆJ'Ê?êy]ïŸ_¬¿ä)™A,5¿êI °N½¿éô›Gð¿á)zLÍ8¿Ø'Ü]¹oUNASNone ?î!PÑG,î?®ŸLÄ:Ü?­êòë1?®ŸLÄ:Ü?îQ_QÜz§?Àd£ý*Yi?ªê
â8U˜?Àd£ý*Yh?ìaS|âçZ?¨ÉU¨Ïe"?¼õdèÅ0?¨ÉU¨Ïe"?î˜Ë[Wa?';Y;o'q?¦sJJ‰î?';Y;o'q4FGL J1409.1-6121e¿Ýmî|M¹»?Àû>û…À6›¾7ÔÀ9!zÈóú8@ «:ðn@(Ôº××Ã?›à¢í€L?¯¼Žç™@Ù¿Š¯?ø¨³‹™Q¿ïÐýH•›?ïðò`Û+¿Ý®êäâ¿âÊâ|azn¿âݹNjÇ¿ãA!"µUNASNone3FGL J1405.4-6119?ÌvõÛ?Ð^MµŠ?èâ\'¾¼I?Ð^MµŠ?w"±×NË?ŸÌÅX7\?ïÐ؜QcÈ?ŸÌÅX7]?㯗Žzß?¶o?Ø Ñã
B?¶o?V¤n2êsá?Tz¸4«µ
?ïô­ÈæŠÆ?Tz¸4«µ
4FGL J1410.7+7405¿ìOj¸éŸ]@Dõ*™0¾À:[rðR
À<ojM{³Ö@ ú'WÛß?økŽXó·?Â_Tä³ÉF?Ñ
ƒÁkÔ@€Ò=Oè@ë3zQ¿ïÿïXz?ïþâ^.‰€¿ÒŽä;(u¿ºÅñ;lÌ¿â²€óZ€¿å"ãÓrÙUNASNone3FGL J1410.9+7406?鹝žêY?À¸ÿARt?ɉ‡ÜVš?À¸ÿARt?ï*`
â'þ?¹\ɋ;­Ø?š³þ£­ÀP?¹\ɋ;­Ø?çTH©¨?³þ
»ß%Ã?ÑWùn­Ä°?³þ
»ß%Ã?ë›)Ƨa+?§'ß"[º?Á"Xåb{Q?§'ß"[º4FGL J1410.7-5945?Ǜ_oz_?ùx"«ËËEÀ9þAˆ`ŒÀ;(šrÝm.@ ¶é—îâ@ît¢iKô?Ç éD&Ëq?˜ÂsªO?ÔãÂwß5@¸áÜò¿ïé|Ñö®?ïól^MW¿çô´±M¿ÞêJa".Ô¿ì	íT+Ñ?¿»P¥	qˆUNASNone?ì™l_4?¹ij'l~ø?»4]?¹ij'l~ø?í~ßsäT1?ÇÝ[]+#?´	`Ý^r?ÇÝ[]+#?ê‡0×ÁØs?¯)8Mné?Åã< øž0?¯)8Mnê?îþÏD°§?"§¡¬õ|? ó´õ'?"§¡¬õ|4FGL J1412.1-6631¿ï—ŽÜÒÄrÀ™V}»ÂÀ9ˆ̼À<Fí$[@'—îž®¬@UÒ°Y?¼€ìब.?Ùlæ³'à@*
4›èÿ@âd×-©?ä9pÏuôy¿ÓkŠ\å´$¿Ø'Äãõ2r¿â¥,¿ü"˿Wz:Y¿ïÿƒ}ùUUNASNone3FGL J1412.3-6635?"'jž?§o&ñ¢ê‹?ﯽ¶U‡ã?§o&ñ¢ê‹?©çx-ÖË?³Žïԝü?în!ˆ}""?³Žïԝü?‰ÊD«k\é?r2yÌ?ï˜ÖíRR‹?r2yÌ&?±Š4â$s`?'º÷*€û?íιc»q"?'º÷*€û4FGL J1412.2-6018?ɔ<­1?ð-}|,¡IÀ9δ#ˆ›EÀ:ég•:H@!1د8D@""úÎg×?ÆÕÿ{&¿ˆ¤ÒK«"Ü?Äñê¾zN¦?þ‰×Í0õÁ¿ïÿYø"'?ïþZxòZ%¿çÊ9¿¿H*¿åCÈü]´¿îä£î‡1¸?ç$¯!k4¬UNASNone?ëOƒ+M€?¾®>'?ÂÁóRÉÿÁ?¾®>'?êƒaä(Õ¤?Ò#Ð~ÐÆc?Åòxo\©q?Ò#Ð~ÐÆc?éHEœK8"?±w,cFþ?ÊÞéŽÓy?±w,cFþ€?í¬Ã²Ï?°5ž+
??·Wâ™âiƒ?°5ž+
?4FGL J1415.2-5550?ífefàX³@'÷na«À:—J4¹À;hoB­úz@^øÓeî@°;Ñgf?×nA§V?âÓïÖ½@¸®$kT@ÊÂOpU¨?ïë°½¢¿â#NžÉ"C¿ç9Á¢w8Ç¿ìŽÜajS0¿ç‰u"×'ù¿×WÝašy¾UNASNone?怷!÷B?ÎÌL]éa?ÓÞþ'¼|?ÎÌL]éa?âj–BÊu?Òµ§]š?Û*Ózkå?Òµ§]š?á^æèî¿?À‰FÏѼ?ÝB2.#܀?À‰FÏѼ?ގ…ow?»4´tØe¬?à¸õ~=HE?»4´tØe¬4FGL J1415.3-6110c?Ñå-ÃQ<?°«ÝSÀ8¡=¼ùðòÀ9àÇÛÌD@ ÄÁ>ND\@ŽŒ:5…ô?÷™»È˜Š¦?ÄNž·Ëß?üG7|n¨@m |ŒÃr¿ë6qY´¿ï;	á€8?æëÂZƒ¿å®²šò_.¿î'lU"°L¿¨k¶B­àµUNASNone1?·Ñ©Ú£?Å¿Z;¸«@?íÊÜD¬?Å¿Z;¸«@?Õ²Õ0b3¾?ךty{=?å&•gÎæ!?ךty{=?ւ·»í'¼?¹çÉx-ñÀ?侤"	l#?¹çÉx-ñÁ?Ô A±®˜?ʀn8È'c?å¯ß'v¨´?ʀn8È'c4FGL J1415.4-6458¿éŸøµÔ&À]±~'­À:"=n€À<Píè¦G'@®:»gʕ?ýlÇß'Bd?̛ŏÝ?áB!"9Å@Uþ9Vc@hZ‡`%?éHtxwàâ¿å©ÚúŒùx¿¶l=?üoR¿Ô /Jpfš¿êyþ(kB¿çy0m†XUNASNone?ՑŸïø?ȞŠþ}›?å70y…?ȞŠþ}›?èg¼²`—¶?Ñw	«{W?Îa
6}¡%?Ñw	«{W?Ùå:µ?¼ŠnGÓê?ãr
uþâ¥?¼ŠnGÓê?ãVž*'?³‰9Uý?ÙßûRêÝ?³‰9Uý4FGL J1415.9-1504¿§(cöÓë@EŠo½'=\À:ä§0ž-À<€ÇÛÌD@e¸Ž|Z?ûWÓ[\G)?ÙoDü‰Rú?×8
2ˆéH?øÜz9'Í@"ô7ŸÔq?ïå' Pˆ¿íAýa¿§Ë.€à©è¿ãÂÜôb=¿æä–bWŽ¿ïÿ´JõǘUNASNone?ïöLÎõ÷?Tïm"*Â?SfcþÙ?Tïm"*Â?ï÷Ìé_¡?k­š|»­ë?PgÜ-@¿3?k­š|»­ì?îó¦^Ï£?"g&mF? ÅšÓ?"g&mF?ï$3ÝëV?ƒ'oÞ'¸?›yœäB•7?ƒ'oÞ'·4FGL J1416.7-5023¿ç|õò(z@$mG8£µÀ9혮¸ÐÀ;øÂ!xÌ@ð·S=êœ@)†@÷A?À$œ—zÛh?Ӆ2ˆJ½@Ø.D¶é6?ø[‡`ﯿÒ8Àr×
¿Ú¬ìݎf
¿Ýê1!5.á¿æ
ÌÁå>¿î`ÊE3¿ïÿÿ&¦³UNASNone2FGL J1417.7-5028?¡5‰þ:´?¢(J÷²dþ?îì®ç`U?¢(J÷²dþ?³4WÜ¿Æ?½kõý)ÈU?í™uh??½kõý)ÈU?©´Bª	­?Ÿ=5*rƒq?îd¾ëÕ_e?Ÿ=5*rƒo?¼ì¸ê'£?žÜoÿä=?ìb|(â»?žÜoÿä=4FGL J1417.7-6057?âñòS1"¿?ÆÊ#åbÿÀ9
>¼(À:G¨=¡K?@$x‰1l‰–?ý
¾4ƒ•K?Á…NÉf»Ì¿©ÂGBÒ/?÷€.>ì?ýîé':,¿‹?à<Û?îf^ê–¿î虱íM¿à³-ߌB¿äÊÜgtƒ`¿Ü'-ê
ËUNASNone?äFat"ì?Ñ_4Y£?×s=Ѻ)?Ñ_4Y£?Ô[wY»×?ׅÁT•8?åÒDS""?ׅÁT•8?åó{O?½èÃ%|â?Õèõ	aÜ?½èÃ%|â?ÕyOêͧ ?É_úä¦ã7?åCX
™,q?É_úä¦ã74FGL J1418.2-5400?ÏòKœòí@áÐÈ0À9ýH"Ô·À;}±CÝ¥@Š0NÒK@i"/?ÒzJHùn?܋AèÜy@èí¢/jQ?ø;O1¡¨?ÕÔ3~1´-¿ß{{áͺ޿è•.enâ¿ëOñå‹	´¿ïûÎ!á|1¿ðUNASNone?ââ$ä î–?Íɸ¦Ö¸ö?Ú;¶6¾"Ó?Íɸ¦Ö¸ö?ɾè&ç¯b?Ίãº¡?éEöF(?Ίãº¡?ևb>o~?¶‹">~~$?ä¼N÷`ÈB?¶‹">~~$?™IˆteG?}Õör³?ï5³¿D\Õ?}Õör³4FGL J1418.7-6110?ãÿ[[ý徿±†SÁžˆÀ8!å±  œÀ9Fì\tu@ör~!Ãõ@¢¦¾EJ?àì){D?ÒXÉûa4Î@
% 8ð?øìWÿÆIP¿ïŒœ[ú?çÃEš>H¿è&@©-¿êcv'-"Ž¿í!­>¼ÿ$¿Ì‡´÷UNASNone?ÌÍÞµš­?Ò¤×ü~-?èþŒˆR™T?Ò¤×ü~-?˜~^ò€?¦´8x†s?ï?_$
m?¦´8x†s?Ç.2yKK ?°†ٛð?ê4sa­-7?°†ٛð?uÃfÜþ‡'?tßÝÊãx?ïÔy2Fò?tßÝÊãw4FGL J1419.2-6029?ê´¼z'@?áöAÛl¢ÁÀ9"›vékiÀ:è‰ÁµB@!"|¨òýä@埱áŽü?سÑÞÚkq?'6¶ e©?ËÈWÈþµ?ü®¨Q˜N¿ïÒÒ4ëš?ïŸÄ UàÝ¿èçˆ9õÅ¿ä"ABÀnð¿å?¼xÁ²½¿íÜ¢ÞìâUNASNone?؂QñUþ=?Ó½¢}?ã¾×Uá?Ó½¢}?åà'ã,X?צï§!k?Õþ>ú9§Q?צï§!l?â4ôΪ	X?½éîY=ã?ۖb«íO?½éîY=â?æ
'9µ
?ÂÅ?nìÈ?Óêû̕é?ÂÅ?nìÈ4FGL J1420.7-6701¿ìLÜ)kÂÈÀ¡©É'†À:ùp™ÆÀ;™oJ:¶µ@=1¦ì@^]×M?ÍmíCdٞ?Μ
!Áñ§@a&Ö.?ùyÕú
¿ì@r`ð…º¿Â¶YÃÀ´'¿çtè?ƒ¿ç ÄÍ¿ëY^@'7|¿ïâ[>ê÷ZUNASNone?ãñX/
?Ë-&Íý>?ØßO¡åÝ?Ë-&Íý>?éãfkí"?ÍS"ì|Û?ÈrfPK¥¯?ÍS"ì|Û?áØ'Æ?¹ì>O½-?ÝÇüO±Ðu?¹ì>O½-?à?ÔJÊé?¸£ðBþ?߁ÐWjj.?¸£ðBþ 4FGL J1420.9-6127c?烈^ÃEC¿Û T¾ôÀ9pAK#êÁÀ:oê–â/5@"Ž™¶Iþ@ð®Ý*?ÍÄn&NH?ªü8ö?è=Pù׳@{…UE¿ïÜ*7áï|¤ËüÃ5?ïø4SÅz¿æn'ûnj¿çnû€"dü¿Úÿr;†¾ÌUNASNone0?çß4kõø?Ìõ-ÙFî?ÐA—(Î?Ìõ-ÙFî?íV/¬Óî?ÊNo҃©8?µN'Ÿq`'?ÊNo҃©8?åa±8Ëö?¿suyµ?Õ<æh?¿suyµ?í"Ú®Z'±?¯æ'"üÀ7?¶é*+rs?¯æ'"üÀ74FGL J1420.9-2431?ã¥"÷6@A¡ýiõÀ:^ÏO^%À<dëÄØí@çÒøŠì@ƞ<–‰D?ŁÂ7rˆ?È'øR¸@_Ô{í·?ùˆ¤~Ïê¿Ô²ŸÅ,Å[¿ág—ô}뾿ݓœº¶¿æ¸]¿xÑM¿äV›†Ù£¿ïô›]i¼UNASNone3FGL J1421.0-2431?íú("×?¬õ)F@[?°/F»ÙG?¬õ)F@[?í>"xIªþ?¿Ó=ågØ?¶\=²¨?¿Ó=ågØ?íF'Ëø¿ò?§…Đ5)ð?µËi :s?§…Đ5)ñ?è]Šr)Ã?­,qAĈ?΋ÁÖ7X÷?­,qAĈ4FGL J1421.4-1655?Û&ï]ÎW<@Dj}¿H€À;'œ%eWÀ<¶´•žbV@"á]¶"|#?×2¼ë®9?âΈ>''ü?î0öã Ì(@vA……@f&ż:¿·Ø\wûT¿ï ˆ¡#і?ìIØá®a¿ïúÕ>
|±?ïöÞï@5¿ç.ÄÑ¢UNASNone?ïéžÜkÎì? 1Ðͧó'?fa#"1‡? 1Ðͧó?ïúö©à;?k璕²Ø8?D%[ô
Ñ?k璕²Ø<?î?M£#»?œìB̞ët?¬%ÍÄO
?œìB̞ët?ïó'd~PQ?e¤a?XÝ7_^[?e¤a4FGL J1422.3-6059?í0ViM¦¿¤Âþ*Æ[À8 6®è¶7À9­O©‹%@ FI²ül"@¢Ä?ò¥K´3xÓ?Ír‰Ië0@ƒðØï?þXËÁ	8?ï| ï
ê¿çú(»
,ª¿ã¼²F+]¿èëë†Ì7¿ìñ"b"4¿×r9Ù?¡ÖUNASNone?ÄÄÕ1‡®?ÉqmQL3ô?êÎʳž€?ÉqmQL3ô?Çoù½Ñ?Ð¥ôÊï$ ?ê$:=Á‹?Ð¥ôÊï$ ?ʑVN‹?±7ÆëüÍ?é[¸jl];?±7ÆëüÌ?£EYYEá¦?¦/¬>
??î˪jk¡å?¦/¬>
?4FGL J1424.8-6536¿Ê‹4'³:—Àâ[úҙ•À:&.gòXÀ;€å¯º@´ºÃ{@ÀLÁy²t?Ù>Nî÷ð?é2užÎ_@p׈§@&{Ÿ^?º,×#'×?ïè¹\­€¿ëÔ.béÚ¿çÏÚ¾|ýؿؓ²Ï˄οåÛíÎmUNASNone?ãSFN‡l8?Ò9*Qiݎ?ÙYsbñ'Ž?Ò9*Qiݍ?ã'ZQ?Õ­"êö?ØÛK÷]òý?Õ­"êö?àj'À‹–?¸Aoügg?ßÉ+°~èÔ?¸Aoügg?ÆHÄìX•?»–'*.¡?êmÎÄéÚ¾?»–'*.¡4FGL J1424.8-8012?ärÎaðdÀ2Q֌i/À;¤š~›çÀ=IÄòø6@Fé—îâ?ÿé={‹'™?ÕªÜ3?ïÿ踻Ð@m$
<ÿ?ý^g×®6¿ç{½ ´ëÛ¿êá|¢¿·†ƒ'F>(¿Ù‰ÿöÅÅ¿ïþ¢½"°S¿íQ&ΠâcUNASNone?Ýé)Šþù?Ñ¢{mZƒà?ák1:€ƒ?Ñ¢{mZƒà?ËÔ°/Ê.˜?Ñü±À#q5?é
Óô
tZ?Ñü±À#q5?Ø w²?º
f¤p6d?ãïÄ|ôt§?º
f¤p6d?¶N­‡èa?¥§D¦î'?í6*OóÝ?¥§D¦î'4FGL J1427.8-6051?ïBò ^˜¿ÂæNh˜Å´À7™ʬaÀ9æ?Pwç˜@,ÚÏÄÎÒ@ùü£T-?´õæ °Ï–?ÅÅxDµ;·@9	ۂr?øÅqœ+?À)nä9P?×´ÿüz¿çÚcŽDÑÁ¿êÊ*ü-©¿åŠØ5¶›2¿à¨<_+߂UNASNone2FGL J1427.6-6048c?·cL¥v´ã?ÄzfEdYw?í–kQ)c?ÄzfEdYw?"%†êëü?«<ïâ¨?ïfÓÏ`¨ ?«<ïâ©?Òþaʐå?µ3áC½ç³?æ€Ïü·?µ3áC½ç³?bä9º?
ü?V¦ŠáÍS?ïíÆEÀò?V¦ŠáÍS4FGL J1429.8-0739?…bþÈ]s@Gìd^NiðÀ;fBÀ<ýÔ£Zã@X6hqÙa@UinX£/?Ô'Ӄ 3?ì|p(‡Ç@[bâMg'@Á*WA…[?íħÈ0†?ïó'?	*K¿Û&ÕøÎ]¿ä՛=ÈK¿íö9ãPœÑ¿ïÁPb#UNASNone?¸íøí',/?¶ü
;3žf?ìâ@âOºz?¶ü
;3žf?Ãðãçý1?Í)Ò,;Ò?ëÇ´?Í)Ò,;Ò?ÓXSÚ*Öw?À>Bî?æSÖê"Å?À>Bî?¬¥´3E{-?•ˆˆ»•' ?î5¤¼Ë¨N?•ˆˆ»•' 4FGL J1431.0-4432?êüjûV@-Ê¯¼ÎÀ:Zy¯ïFtÀ<"¢"=_@ˆ´™û@À#Uož?Òø®6Ý?ÄïäêOêy?òåQÉ oâ@ÉÎÖ俾šP£±uƒ¿éÔÎX¾7¿ä+¢zé«*¿×")ÛE¶n¿ëQ(¡´Æ¿ïñwÁØ}UNASNone3FGL J1430.8-4434?ï󚖾Ê)?Y|
ŒØ?XÊ҂k¯Q?Y|
ŒØ?ïûò!£8n?]œ¾"NS?@7ysI}?]œ¾"NQ?ïmç}jb?wUÌæ\«?'CR½³ž?wUÌæ\©?ïçÕ+²?U0Îa-?hæ*ÔâM}?U0Îa-4FGL J1431.5-6627?¾h"×ukÀ	‡Æ2~ØÀ:CÇE¤NÿÀ;±•ìeïH@äjÔ4J5@—dj㣩?Ï_T¹À«?Ì!^IŒf@BÌÛæED?öAkBS^?í:1…ý¿à¾Ý®‡¿èDƒBL"¿å"M!pèö¿ïÿò> w?å6YX`êUNASNone?í™åÇ꾇?²ìŸòdŸ?³0ÑÀªÈ?²ìŸòdž?ën;d¨wh?Ê›[èô?ÂGm^"^?Ê›[èô?æh¼Ø%ûô?¶·¢25¾2?Ó.†O´?¶·¢25¾1?âfËê,?¹[fЂ\?ÛÏ2h+§î?¹[fЂZ4FGL J1433.8-6357?îÉÐUÒÌÀ
R˜˜—;À:áÍ:°ÕöÀ<§³Ó׃	@GpxŽ@¸îÿ&¼,?Ö×.Û4ă?ïÿ—?LF*@
φþŒby@6Ö)—Óò?îª÷?g?ïä;û…G?°1æA'òa¿çx!m
¿íñ܆~3ã¿ïÿ\‹/ôUNASNone?ÚýV8¨É£?Ëo]kÔ@?âT㫛/?Ëo]kÔ@?ÎlU£î¬Š?Ò4j56Â.?èdê—TÝ?Ò4j56Â/?Ú£	é{Ý?½Â'$œí?â®{B8?½Â'$œí?¢UâÈ£‡?'³'^ó6Î?îÚ®'ÓuÈ?'³'^ó6Ï4FGL J1436.4+3900?àèV…e@PG͉‹.À;¥á¨&$WÀ<ë]à…ç5@ `¾$ƒæ?ÿÓ¯tÍ1w?ÎÆCÜ"Ö?¡SÀúå?Ӟ¤Zè®Ö@3Ý	°Øпëkô0õk?ä(½ž†"X¿Ü³T€µÇø¿å†žEÑ¿Õ½ÄܓiT¿Ó±<MŽ(LUNASNone?ï÷f™\?RÝv2>j?QÕ3ÀÍHP?RÝv2>e?ïü—G?T'ŸÓ®B²?;GíÇ(_?T'ŸÓ®Bµ?ïÈ	ÿ­½W?|Ïí®%!'?{û)!Tp?|Ïí®%!‰?ï杚Y\Í?Y"ûTú?ibe¦£2Á?Y"ûTú4FGL J1438.0+0219?ÀJó³<Ï@K6-œñ<ïÀ;MÆF ÎAÀ<¦MÝÙe@4œ´V3h@Y¨Íê>?Ñö«XþÒ?ŊnÙQ•t?ïXBKÔê¨@¤–^PÃ<¿íN¶È¥ ?ï÷䨋¤ä¿ç‡âg^3¿áv"@Áç¿ä©Y?·P¿ïڅAÈÍ9UNASNone?ïú`«š h?BúÍÿ2Á?F}Q—~]ì?BúÍÿ2Á
?ïü"v9mü?TÉ?^ºÎY?;ÜN4˜?TÉ?^ºÎQ?ﳒ ÿý?'¹R˜5EB?ƒWÿÀä?'¹R˜5EC?ïé¾+è5?VÍÔù ÷?fAÔøʊ?VÍÔù ÷4FGL J1439.2-5142?ߤú©Ê@ºø>jžÚÀ:"…fîÀ;¬ÿðÇô@ìüÝ5М@®}Vlô?ÐsÀA#6?È
‰Æ½¿?úRš×‡;?ýàwÇaÓÛ?¡g"@
ƒ™¿ç<ž_æð¿ã«4–àµ¿è«e©¨–¿ïÿúVrÓ\?Ó_o|9·\UNASNone?ìÐn‹™ã5?·"²'«c?¹|‹£0æO?·"²'«c?ëЀâkxX?ÅìI\£À?À½üvR¢?ÅìI\£À?ç½Õ‰Aì{?¶°_Ø/O)?ЄTí|'
?¶°_Ø/O)?ë^e‹Tž?§F^ғ˜?‡ŠiÒ­‰?§F^ғ˜4FGL J1441.4-1934¿ê" ½ÎèT@B¦µ(À:ñ"Nü½À<{Ó"Qc @!-"Pª<?õdãåFn?Õ3_¿-R?à
¨š¾\È@"•ƒŠcœ?ôùkjÏ?½|­_I<¿ç9äàõ?ؕAED­¯?°O\8û¿ÇRl´^@þ¿ïýʀÂ2?UNASNone?î¹gZΤf?©4Ü믂é?¤iŠS¹ž?©4Ü믂é?îPVÈäN?¿áø|¯€?ªú"Çq»?¿áø|¯€?í"ÆöL3?¦åôìBH?·ÙÈMžh?¦åôìBI?è
öÊï®?ºûäѲ1g?Ï÷Ô$ÔAH?ºûäѲ1g4FGL J1442.0+0732?Ñ0vîx@L£ä`gHäÀ:݃¡àøÀ<o?v7"Â@2G?ڋ|@aÓÅ'j?Ð1¾"ùò?ÕGfÿ1?ÿ0	}WC´?ûQ0αÿ?ï¦ÿ]ꏿã°É–·g
¿á™î=µÃ¿ã–€À.Ù²¿ê_`—Ì:¿ïƽ FUNASNone?îƒ×Æ&¶?£1˜kÌ3Õ?§Âƒží"¢?£1˜kÌ3Õ?ë–ɪŠí)?Å« 2üÍ%?Á¤ÙUÔK]?Å« 2üÍ%?ëà˞(?¥Ò¼®kÂ?À|ч¿_ä?¥Ò¼®kÃ?ã¸Ó€™¯P?²B®	€?؎XþÌ¡^?²B®	€4FGL J1442.1-2800¿âs'ÿÛó@<ÌRş±âÀ:|غ@ÙÀ<A˜ý'gv@éN
'@cq|D=?Ƒf"ÄJr?×âûã:Í[@¶ˆ7q†U?öKÐc\0?ß¡—_,¶A¿Ýœ"`IÁÀ¿æ¤ªÚ3½¿î»CÝOÒ¿ïù~¿\¢¿îvª¡~ÀOUNASNone?ãâp˜CùÚ?Ñ^
×љ¼?Ø;ÏxN?Ñ^
×љ¼?Ôý¿ŒH?Ôð ?;?å w¹öÝ?Ôð ?;?ßošÏå»T?¶L«²è•?àH2˜
"V?¶L«²è•?·þ#¢¨?žð@:;¬Y?í;‹¿j?žð@:;¬Y4FGL J1442.1-3707?ìxþS剨@4­3;–¯À:ÏeóSIÀ<"­Ù©T@ 6šn*Õí?þ'Xœ‰8?ȁ'ºýíV?ÁmhxºPô?ù¿ë¨Z&½@\"H?ïëy@×æ¿âúò¿Ðû¿à¥lZþ¿×i#°q¿à™RÓº}¿æ±·û"pUNASNone?ïóî'–;?`­=	à?Xü"ÚӇÚ?`­=	à?ïâò³±B×?ƒùROïø?m
LN½)1?ƒùROïø?ïÜËRÏß?wts¦þ?qšV˜pñ?wts¦ú?ï'Ð÷h3Ï?€ "-Ó?›áù†;?€ "-Ó4FGL J1443.7-7037¿àUÓ)jh(À#‡ãÑÌÀ:
j»_¼ÿÀ<¸{0œ@rôf¹@ó¢#«×?ÁDyA_ò?À?PøÀñw?ýò–³5L@ÙÌ¥	º>?ïáö?6÷Ž¿âÅõåÊË¿ä_²?¿à²üÁ‡¿è½/Á
ÑпïÿüoQÇsUNASNone3FGL J1444.0-7033?ïp".qJ?£¶Pâ,?'üš1ÖÇ?£¶Pâ,?ïØh`zÈ[? NÖ]h?sËÏ›ҍ? NÖ]h?ïξZr?–Îêõ¾—?œ(4¿qÝ?–Îêõ¾—?îÅv'5?ˆoû	ü '?¦ó¨–ì®J?ˆoû	ü &4FGL J1444.1+7601?È»¡¼(@C˜P%"õÀ;›Ãèø|~À<÷Â,_Ú@QRÖç'Ü@E]Ø"k?ÔZ^ï®?ËC扷N`?ï>~jê?þÅúˍ³¿î¨f»ö»´?ïüKuIX9¿ÔD­®úSï¿äÏBrì1¿ã1ÿ÷œ"0¿ïý³¥ÝuUNASNone?ïà*'‡f?nÌÐ%J®Ð?oÕÿnx˜þ?nÌÐ%J®Ï?ïîí&gð?}öqÄJ½3?a٘ãW?}öqÄJ½2?îÃñ¢Ë.3?—q†Pî©?£ÀåÓM×?—q†Pî«?ïI£\ÍO{?ÖK¨ó?–Ë"fV°?ÖK¨ó4FGL J1444.8+3645?ä‹?àÔ@P
·AJM+À;	5œ™ÿÀ<r@žUÀý@xi^hk#?üŠÉ‡î"?ä!j³Ó?è)¬¡´N@8³¥´Z@͓´RW'?ïh<>õ‰/¿éHQ¨i@5¿á¼ˆ¿îm¿íQ‡aˆ±¿ïí•Ïà}"¿ïøtP3ôúUNASNone?Ò6'Û?"¡)«?ŒPKr[‰b?"¡)«?쀹»KÎõ?ÇíÜU7?»ú2%¡ˆ\?ÇíÜU7?쌉[H?¤ÓbXi®?»Ÿ³•%Å?¤ÓbXi®?åƒ
³ ?¼:º>Hï?ÕãÈùê˜Â?¼:º>Hï4FGL J1444.9-5939¿ìTÛ¶Š"?½Hô‹(À7à°.0"óÀ9Õ~;oA×@ס–¾@»œ=¸È3?»ZÀ?ö?×)±>y@ Vlô!?÷ɋúŸ™?î]/Ÿ¾w¿ÎIÊäÀ3Œ¿æä:og—¿ë^u×±ç¿ïÏk¾Td¿ï÷ú"‡UNASNone?µñD˖ׄ?Зx+¤$ö?íA×f%?Зx+¤$ö?oPØ¿èhù?v–"ÂÔ£Ã?ïà¯'@—?v–"ÂÔ£Ã?«-î.ÏÎh?¢æ3œuÖ2?îM!?¢æ3œuÖ1>󍶬d¼>èð8AU?ïÿØ䒧ã>èð8AU4FGL J1447.4-5757¿ëj(1›§?ø^Ç»ëÓùÀ8‡¾[ðÁŸÀ:¼ÏJ«@j33fà@ký."h?·R‹íš<?ÜVômû†@û*ÂKi‹?ú"ŠÑ¹õ?ïõÄ"`¿ÓÏ© Z8¿æMOÿqº­¿ìzÆ:"‰¿ì¨õŒßvó¿ïþp]áÁUNASNone3FGL J1447.3-5800?\žÖñëá?^·ƒ»Ïït?ïñ°"‡
{?^·ƒ»Ïïs?zÖ·Õ3?Ž¦ç"³Œ?ïÊSñؐV?Ž¦ç"³Œ?¨MvS?Ÿ^딫?îN[.X›?Ÿ^딫?$g9|'EÏ?.9 §uÞ?ïþ¹Œh7Û?.9 §uß4FGL J1449.8-5923c¿ï[UÄNI?·a» ™VíÀ8¨f±åÀºÀ:B†Î»ºV@¥{Ð'@jTà,%"?Á¾x÷¼Q?×Xö;[á@•!4y@¦ã™—ì¿Ý'ހÔPп£TcÀªæ¯¿ÜßLÁ¤¥'¿éFÝÕ2ÌÜ¿íÏr™{¿ïþ€£ÿN)UNASNone$?€Sʑ?™j–êøçÑ?ï¾³"Õ»"?™j–êøçÐ?£N˺õ
j?·,Ädøw?îËDP¯Z?·,Ädøw?™©;G!?'†(£àÚÅ?ï2¶%Æó"?'†(£àÚÅ? kN?Œ¥¿2£ò ?îùO›žÏ?Œ¥¿2£ò 4FGL J1450.8-1424¿ã3Ô7f²@C®Ûʖ'À:ñ9>/HÀ<«©Ìíƒü@¦o;÷ýÓ?ÿ	‡ƒ U?ËzÆ[¯S?àšIÂÁ±@b.ä¬?ýZæØñ~?ïÿ•!îZ¿ß°nh@†¿Ðä¶Î]Ç¿àd"‰—Ã׿ïÿþó…õ¿í<¢¤@UNASNone?ì:ْý®?¿SÐ{˜u?¾)ã3h?¿SÐ{˜u?ÇB~õ?ʈ±:½Ö?ê;¯`B¼\?ʈ±:½Ö?Ø^´7?»Âä-ž7?ãóPý%är?»Âä-ž7?ÈBMv—yå?©5õEE¯b?éïl¢Z!‡?©5õEE¯b4FGL J1451.6-3726?ÙäԊƒŸ@3‰ ÝDÀ:†\ø(›*À<*ÐíýZ@Ÿ¹"uö§@ž¢ûB+?ΏbÞòi?Ø}VÂÚZª@'!ý€É¿@~AÉùÞ©?î¼´áɉ ?ëmô?,­¿ÚLǤùv¿è<¦ÿ³©æ¿á+þöë"H¿ðUNASNone?çŠÊF>î‡?È!=™šÂ?Ðêks'"ò?È!=™šÂ?â‡Ë¬@ô]?Ӑcq¹—?Úðh§~F?Ӑcq¹—?å£Ç<gé¢?¸sL5.í?Ô¸q‡0,»?¸sL5.í?à6¡>Ê?¹©ÖOÄrv?ߒ޽ƒÚm?¹©ÖOÄrv4FGL J1452.0-4148?㳘à*M@/J^±¬À;$üȼÀ<ƒ|Æúû´@ Êì=ÖOX?ÿ´W£U?Çú–È¿\…;T%Ï?™ÿÑån@T$Ñp |?¾=‰ÎJ{N¿áû¶úÓpU¿Ú׶_Íðä¿ÜsÿÁ–¸¿¿Ý<ñ¢ðŠ¿ðUNASNone?ïü>a%%þ?<Ùàg©¿o?>öÖÐþ?<Ùàg©¿h?ïüÇM)¦?^IzÍ6Á??ÉŖ²Î$?^IzÍ6Ä?ïä5¨èy?súKÙ)?kÊãW‡??súKÙ+?ïàˈ´ïn?X	_y}?o4wK'þ?X	_y}4FGL J1454.3-5551?å½Åo1¿Ç@äI:ÜtàÀ9ö¢ñ10$À;Xù"«ô@"£ÊŸöÖ@zh˜q?ф}*[?Þ|´†"éß@Œûü@_œ"JÐ3?î…ëÃ¹ÿ?°Ý§Û¦¯¿êóæasbx¿éÙ—â¿ë
´Û¿¿ïýf],+UNASNone?ÒÐ	Ôd?Ê¡óI?æ—ûv•öN?Ê¡óI?Ð̃Ù6ª?ÏWæÒëf?百|"dª?ÏWæÒëf?Ù¿0ȧ?¸
T3?ã} gõ¬?¸
T3?ÎcrÈub?°#šœÂ3z?èg#
â¨?°#šœÂ3z4FGL J1454.3-3946?ìX¾ N@1<¯bk/À:ϳô¬æÀ<̙¡&@ýˆf# @ÿMzÝð?Ûô°@¥¾?ß?p\‰?ø)&i÷@´^»!S¸?ä»!©ô¿éî4Ïëe¿ãç ÏÃÍ¿ïÿÿ>¹ú?ïÿ‰ñÇ®?ã–!‰"UNASNone?館ï4‡?¡Û

ǂ?…ùÔÄ2ÞF?¡Û

ǂ?ïˤ§Nã?¤‡J7•žÓ?z-ô¬XÉ?¤‡J7•žÓ?ég	yb}?²Ïlân€)?ÊcÚÞv?²Ïlân€)?ïéc×"?kx—¥ï©Ù?fœ(ðïݔ?kx—¥ï©Ö4FGL J1456.3-5419?ﮜcB–@ي¨exÀ:Symª'†À;Ôj:0}v@Ið<h'@ž˜ÜÛ7Ê?ËOž"ë<?Ú6=©¯@}¦Z?þ)Þb÷F?êQMÀR@¿çœ'0>Œ-¿á>ƒö¿æ¡o† ˜'¿í«a·€	¿ïý\á0UNASNone?ΗfŸ??Ä(1OS+?èZ9f~Ø0?Ä(1OS+?ÊOÔԁþ?ÏU'†Ê-?él
úÊ߁?ÏU'†Ê-?ÒE6)ø(?·±Eª–Þ—?æÝdëóì?·±Eª–Þ—?¼-`ƒ©´? (	;Ëk.?ìzSÊ? (	;Ëk.4FGL J1456.4-7129?dú»Ÿ´DÀ&`®–À:ðª¦1W'À<m¡â=wZ@m®˜YR­?ÿ¶JêßÝ?Òk–|ÚÑ?ØEAþ}@pë?~›@uVSsÅu¿ïýРkð¿?ïÿ¶~¬®I¿âå{ð;g¿Ùó:à%Å¿êmbnŠ!W¿ïþÇ1¾UNASNone?ï­ôå-Ð ?…aЩŽm?"'Æ´‹ø?…aЩŽm?íøÓû‹'¶?¿ Ã+E§?°9`#£êC?¿ Ã+E¨?í.•ãö?¤
g²}T¯?·V‹WàM?¤
g²}T¯?ëQ€öc+?ªÉ*â?¹ü&rV?ªÉ*â4FGL J1456.7-6050c¿îrH1øžá¿ùqÕëYÎÀ;e߅65FÀ<1vßZn@&£¨žð?ó­Â*²[1?Ê+?Éą¿¾Þ㥬Lz?öy^«‡ç@Êò4:o=¿ïÖHaÇó?ïí,•<=¿ì÷³•Ä"¿êzàñÇÙ?·4£ ®Œ¿Û­ë=ÑUNASNone3FGL J1456.7-6046 ?ïý¨ºÁ"?>MÂ5Â?2º)÷^ï¤?>MÂ5¼?íÿ¸_ðî?ÇU&Ù?°'=x?ÇU&Ù?ïCHŒ ì(?ŸÆþߌF?—–î{âzþ?ŸÆþߌE?ï:	ÖAžà?¡Dߦ } ?˜¾Å7Ì$?¡Dߦ } 4FGL J1458.8-2120?è°+sÀ:@@H‰ÁµA–À:eJýTTÀ<Ê8Ö?@ªqùílU?üäœ,ý?Ä·.jv–_?Ûë<äâÃ.@à8ýw"@p^ùÞ?ú¢É¿eQÃÂ)"¿É|ƺš¿ãÕô~A¤e¿ë6zæP+'¿ëü?¶Ï4†UNASNone3FGL J1458.7-2120?•Æç~ÔÁ?'+àåðš?ïWaÈÄ	Z?'+àåðš?Ô.|\7?Êú|Z7*Š?ëô`èø²?Êú|Z7*Š?Ÿ<Àž?'‰'ŠÑ®Ë?ïß/!ü?'‰'ŠÑ®Ë?ÉÌʍ™_?«fÁ¹é?éŒÍy\™¨?«fÁ¹é4FGL J1500.1-5846?´ Àê1d?¶j#¤
ÖÀ8®n‰J—À:'¤ÑÜF@¶ßªõâp@7րªµK?ËØF=&&/?ÈL«êªr?þ¦îœ*m'@%ýžü¯é¿ë¶D•[Fx?ì_>Sù¿è2í"ñÚ¿é¹Õ䣃'¿ê1y¿ß~€¿á´¬¯öÓ1UNASNone	?Àüª*½žv?Äùâ¨7?ëÀÕuP˜b?Äùâ¨7?ÁœyZ'ëK?Ì;Øò2Ç?ë˜á©[E-?Ì;Øò2Ç?ρ•Æ[¥{?»ïØDáÐ?蚎i¡?»ïØDáÐ?Õ ms¡z×?«6Ýx¦??å/ÉF/B"?«6Ýx¦?4FGL J1500.2+2640¿Íº‹ä¾@N®"î9.À:ìðó®À=á{°z‡@ï¿ÿ^ðP@^@ÈG,?̈ѠF1?ïÿöàœj@Ú­æW¸N?þ äßh/ê?ïàÇ ½û#?ÖLòãÕ¨¿äáƒÞFqÔ¿îö'"׿ïö4osUb?ÃVú£ӀUNASNone?҉Me?›É?ÑB4ß½±ø?æ»YM`2?ÑB4ß½±ø?"êN³–Ùé?ž±pë?ï`­ŠcI0?ž±pë?Ónö"[ú?²,ö´H?æ~ȄîÒ?²,ö´H?VýºíÝ
?H@»éen?ïôõ"‰?H@»éeo4FGL J1501.0-6310e¿î¾UFÀ Oœ'rÀ8AðáyÀ:c7ݼß@:<§P;'@¾¡žJÙB?¹ÑÓFäjù?Ò(ÝÚ;JY@Âl~®[È@ؐ$zß?ïÿA>8ÊÍ¿àzjÊy5v¿Þľ`xe¿ç§(bõ˜ž¿äQ¬šþ¿ïþi'O¦UNASNone3FGL J1457.6-6249 ?ÄÁ»óÚ?À.)Y@<?êϑ	€?À.)Y@<?¸³§RA¬?Â-íXa?ì鐷Ê?Â-íX`?Ò¡â«Ö}?µ°×£‹,?毪|"Á?µ°×£‹+?ºQVļh? §@åH=?ìµÕ?'hs? §@åH=4FGL J1501.6-5236¿²•3$'F@g¥ßøù|À:fž—/\À;Š]«¬Á•@®šǦ@ßæՌŽï?Õ/`àëgÃ?ãwÛÈgã@{6½+o?ú"1Ó·¢™?ÆÛ˜ÜZ^?èSðlõÍ¿åõJÖ½ç¿îˆÍ¿ì³ß@ñ^¿ïýZØ®UNASNone	?Ø^Ð`}…¬?Ðu¤ˆÖ€?ãЗÏÁ=*?Ðu¤ˆÖ€?Éãav—Ç?͎†°•T?é¹Ç'¢Z?͎†°•V?Ւ"¯çBœ?´B[ƒDzV?å6î¨^²?´B[ƒDzV? ÕóGÅGƒ?ˆð‡ÏÝ1?îò Ëƒ«ˆ?ˆð‡ÏÝ14FGL J1502.2-5933¿ªâ3Æ»¿è×z:XÁbÀ:6›X¶z{À<nšèN3@ìÖæ(ß@yn‡PÂ?Ó|_…?ïêÇß}( @·zâm©@÷½Ñ²9Ï¿ïò¶kawê?ïû|ã€m¿Ü‰¦qï0¥¿á?ÅGMƒ¿íûª€qªg¿èÃà•®UNASNone?" §.è|?¡9˜{¸PP?ﯡcD^?¡9˜{¸PP?™þ`m?6?«÷´ïklÁ?ï3€ü–?«÷´ïklÂ?µõÖ,y1?£¾^k*9?íAE:pÚ?£¾^k*7?‰0be&é?wvEû!)?ï›>vkd[?wvEû!)4FGL J1502.6+0207?ïø¢áÆpK@Hï? §?uÀ;P¤J̓¬À<œ—w€j@ V"‰Š,ê?þ'ê–o ?ÐùùJ÷?ÃígaŽx?óy¡â=wZ?üjÔ²t[ò¿ïù™~Á¦ÿ?ïÕɕà§u?ï(¥:·‹ó¿åêa2Iÿ¿ÝŽè%Bڛ¿äƒÎSŒðUNASNone?ïûÙEîbf?A·¶Þ+]?@šèFvfT?A·¶Þ+d?ïë`¥³RÉ?Ëƒiœé?dŸZL­8N?Ëƒiœè?dYôÃ?""¼ 6?ˆS&é'Ïi?""¼ :?î¦tª=¥?–A"¨~Á?¥˜µ\%®e?–A"¨~Á4FGL J1504.6+4343¿Ô™~`Ÿë@MAtNƒÀ;±ôr{HÀ<æ¦qq@!:¾lâ¬?ûBr5§º?Þ%€W©4A?Á°ûàá'?ß¼[»g @^"'GA³?íîÃA³©¿ëZ=c7ݽ¿é•¢:Å?¹yÿöDëB¿é™RÀ—¿Ò½å=ÜÚaUNASNone?ïõÇ7OǓ?XG¶ª¶+¬?Tq'`pك?XG¶ª¶+±?ïûÿ!h<ü?b›NÑ.oS?@z_?b›NÑ.oQ?ï'ÙJfI­?‹gîÏÀ.h?‹I­fm"°?‹gîÏÀ.k?ïâQí¤æ?^äEG­!è?m®ï[3?^äEG­!î4FGL J1505.1-5145¿êQDóÌ)`@WbØ<l˜À:P•,L%À;'(mÝS-@A—ȉG@R.»Õ-Ä?×ìe$?ãrl™†Nc@Æ.Z†^S?ý«è¨ˆË¿ä"œ!´/È¿ã)¨¥¦V¿â³CÕAæ¿ê…AÁÇ¿éèv¬.ǔ¿ïÎ0»"¦UNASNone?¿U΁±?¾ê¶ÏÐ?ìuF/ÉÑ?¾ê¶ÏÐ?ÓPÄ$3?Ñ(!DŽ—?æWýýíæ?Ñ(!DŽ—?Ӎ$8\É?´î"Ô[DH?æ9mãѹ?´î"Ô[DH?Ö¢CÈEËÕ?¹o,ÖN‡?ä®ÞÝ?¹o,ÖN‡4FGL J1505.3-5852?â·:Is*u¿Ø#dn•À8\ëÉVjÀ:ïLS•©@ÊþOPË@l»Ý'@/?ÐLÌamb?Ú@Z£'®@ Ÿ°4?ùB)Æ"¿Ù¼sƒ…[¿éyq%Ú¿æµ^ñýÞ¾¿æ~˜÷³*d¿íú'
‹þ¿ä8*lUNASNone?Á-7'Ь?ÂÛ~ÇÒ#?ë´²6Õ?ÂÛ~ÇÒ#?ÐU™ÈzÌ5?ÒÏ<¨i?çÕ3™æ?ÒÏ<¨i?ËÑ$+ô½¢?²7¯¦KӒ?é¶õИ?²7¯¦KӒ?«çÞ2`V?—zû€ôé?îA'Þ)ú?—zû€ôé4FGL J1506.5-5708?ï÷d0I?𻦺Œ¥À9*#²Œ¯¦À:ÈÃB	Ì@ƒÇaÓڈ@@ÝûÉ9š?ÑP¸_˜1?ÔÄÃÿž±@FGwÖ@°s#Ž$›?íçòpËD¿ßÁ‹›T.Ö¿äD8¿HB¿âë7@¿ì*í+&¿ïÿ·`)
UNASNone?ØòÆé7
©?ʉvG'›?㆜‹dy+?ʉvG'›?ڀ :âUÔ?Ô|úl9š?â¿ïâŽÕ?Ô|úl9™?Õm£yh%?¶D‹Bُ®?åI.CrËî?¶D‹Bُ®?ߤu}8¼?µ_ý
)°³?à-ÅA|c¢?µ_ý
)°³4FGL J1507.1-1901¿î)ôtÅGº@@©º^5?}À:Àh®?CÀ<)Táä·@ê+ÌâqO@œÃB	Ì?ÊK‰@[￲fCUë?è8)Âq)8@›oðRãÓ?í-$%y6M¿ê"`Ø\ù¿ì>â=ø¿Ä`‡êš"¿ïé¥J§Ãÿ¿Àø\È_UNASNone?ïìŒáv³?n&û"zÚ?cs‰Lï¶?n&û"zÙ?ï i™{Þ?¢)['1 ?‡å™¡;ȋ?¢)['1 ?ïYó?´»(?Ž.Êøeý?"Á˜	h›?Ž.Êøeþ?ï³cs'þ]?|Ìúæ(ªá?ƒ'#6hÇ?|Ìúæ(ªä4FGL J1507.9-6228e¿è¡KuÇ}À
@$ À8èO,ý"À;`CނØ@"`¼x{?û÷Oݍå0?°h­é\Ð?Uö´9És~?îz£q+3?îã!øÎ2¿ÂM%²—¿àWÕ©ë u¿Ú~½ÀjhÔ¿ÖCÐú®ÝN¿Ó"j@ºˆUNASNone3FGL J1506.6-6219?ïÞ¨ª×e? $ÃïïU?p«üª"LÍ? $ÃïïV?íGã_,?Æß TO¢ä?µÀã}¡?Æß TO¢ä?î¦ ¾®ü?›ýÇKêóp?¥þdK?›ýÇKêóp?âώ²Ž<²?À+OV©´ý?Ú`âšã†š?À+OV©´ý4FGL J1508.4-4817?ŸI÷c…ôË@!)éBNYÀ:·o¿«|À<°}á­/@ˆmm–±@!#=ò©Ö?ØU-XþŸ?î┵.J–@ÁÀÊ`@ùï‰:Pß?îïŠ1FÉé¿á{À nŸñ¿ç³"âz´¿í³Y(B¿Ð†0[<'¬¿ïÿæŸÜ©ºUNASNone?ì)S깪¼?Áÿ|D½Z?¾µ`ª2ª?Áÿ|D½Y?䕑be!?҉›{9ðŽ?ÖÔÝ;5ó¿?҉›{9ðŽ?çvÆQª£W?µj2K¥?Ñs\ª¹R?µj2K¥?ã#F‰æ!?ÃØ7"Y?Ù¹rì3½ø?ÃØ7"Y4FGL J1510.1-5750?ïÅv'qa?É7ÑÌÀ8àpØ°/ÞÀ:DÄ)B@ $ÀS @ZQ	Þ?Â*2	h?Ѐ{zõ"—@	—ZYè©¢@0oz¿ïÁ­)«Ë?ï'ÄþÍ%¿ã ®@š¤Ü¿åxÜö¼6¿êk7@7¿å®7¶O²ÆUNASNone3FGL J1510.2-5754?ª"mA§h?¹6oWUFl?îV¹+åŽ	?¹6oWUFl?š£@'øƒ?¬^Ž¼.?ï*ç-ûh<?¬^Ž¼.?½øf€L?¥žÑ©ËW?ì@ÿ=³/ö?¥žÑ©ËV?µž,F}v?¬v+€ž??íL:w0Q<?¬v+€ž?4FGL J1510.9+0551?î3é%(t(@IM½ƒƒ­ŸÀ;IÝcpÀ<©7Ó«ä@ ¢§>H?þ7?öå?ÑWó;Ì^é?Ï
ŸÎ@ҘÀ¤ @¶ÙTD¥Ì¿ïùçýÕ®H?ïþY6Òúä¿Ø^m^'Rª¿âQ"ŒÂ¿×ÅÀÔqý¿ïüe"´UNASNone?ïó1yW?X,Œ—˲?YÁ
QîÔ?X,Œ—˱?ïîqò9y?ç\3Ü>?aŽà
ƆS?ç\3Ü>?ï¿èâüm?'DÓíã"?œ(ã rj?'DÓíã•?îÙ@Œ%ÞÅ?¨5'…Ñ?¢k÷=¢©?¨5'…Ñ4FGL J1511.2-5803?ï¼B‹£.¿¯ù ?{À8u–†¿¢BÀ9Ó²ÊÃQ@ ´<[Ðá/@C{~% ?Ö_þ"/T×?ÃWÿJ?þm…É=?ÿÂ+[xv´?éu^C,P¿é‹^e¿äˆHn-Û¿êÒåëÃº¿åm$€½ÕŽ¿ê¬ÄÉ$¢UNASNone2FGL J1510.9-5808c?×m§
ƒ+œ?Ò`8†Æ?äI,y>j2?Ò`8†Æ?ÎÈ%å-j?Ò<³±‹Õ?èMö†»t¥?Ò<³±‹Õ?Ô*}¾Œƒ?Ák±^µSÎ?åêÁ ö9¾?Ák±^µSÎ?¼é‡Ó¯ø?²?¦Ž2?ìoÂÏŠ?²?¦Ž24FGL J1513.0-3118¿åæÊMj+@6ƒõ@‰]À:Lm)ÏÀ<	Ä|œ2Ñ@ĐlIT]@Ý{~%ŸÍ?Ë®ýmS•?ÐÇ`&[^@Š#ÚМ@z6‡¦}?ë«6D_«a¿Ø	Žôúé@¿ä4߅·¿á'¼<[Ðá¿ïÿþ½à ¿?ï.°'kUNASNone?çL "‡Q?ÅÔV{î­Z?Ñf¿Óºñ^?ÅÔV{î­Z?ëܐPČ\?È4ƒ1(C?À¾¼íΑ?È4ƒ1(C?äf;?åTC?µb<`°?×3‰€5W{?µb<`±?쒍›BH¾?¥¦
½=2G?»k"%íº	?¥¦
½=2G4FGL J1513.7-1519?æÀè¾G@A¢´A»Œ3À:õª®d,À<§)¥÷ß@_JÄIpŒ?ÿ×E|Y?Évz° F\?ÙÞš@
•ZÀ?ö@›R}PbÄ¿ïþÃT~–?ïÿþªJl¿ÖÔ]Ofo¡¿Þ´Þ. |¿êÂf͓œ¿ïñ.á"ÚîUNASNone?æ\|÷ï?Åi¼î@SÞ?ÓFá$?Åi¼î@SÞ?äTíå¿}?ÓðÔÞâ )?×V$5ށ?ÓðÔÞâ )?ß'Ø¿já?¿H˜Óѯ€?à}>" J?¿H˜Óѯ€?ÝâíQק?¸WúØÍQ?á‰s×,?¸WúØÍQ4FGL J1514.0-6240¿×©æ6®ÀÂ6ŸÏ=ÀÀ9Š»¬éØvÀ;6Û¿®×@S«šMÀ@WGC¸?Çê›ê¬²?ÉpNœ›+À?úzÞÞGH"@w9ÝÇEú¿ÓwÕd ¿ÖåoÛÛ£¿çUyC¸¼u¿ì"RÈú°¿Ôåî|b¿è©xŸNUNASNone3FGL J1513.8-6250c?ï!OnïQ?š¦kèß*?›Ö2"ß?š¦kèß*?ïú«¼H?k~ÃD²k*?ESßó1?k~ÃD²k+?ëjü¹š?ªÛ(j´Ço?ÁŠWü
ž?ªÛ(j´Ço?﬛Z6>Á?u%²
Ñ?"Ù)rpOÔ?u%²
Ñ4FGL J1514.1-5805c?ìÑ6''g ¿Ò"á#
À8ìÆ)wÀ:I¶>ëÎ@ É•½@Ï8ÅCk?ÄWŠ@
\$?(žÒ
?Ñ(@;Œ'?째Ex§¿ï¬^BUÿ?ïIë`á—4¿áu¿¿èŒ'Jÿ†¿àé¦A¯(¿æ֒³ÌJÇUNASNone>?à¸;–øD?×M>ö,?ޏˆÒÓ{?×M>ö,?ãFwWÅ{c?ØÒxRgE?ÙsPu	9?ØÒxRgE?àY>æk?Ãt¸s@Îà?ßM'3ß)Å?Ãt¸s@Îà?Õ5gV‹FÒ?ÁÄ~Ì^™?åeLTº\—?ÁÄ~Ì^™4FGL J1514.8+4448?Øò%~@L5BÙÏÀ9¾E	Œ³À<1¹[ÖÀl@
61u@­Ò^Ý?µ•¬O(Ý?ÅQî׶@Pó_ތé@ó̕ðB?ê_'Bd(Ÿ¿à¥è'
è¿âý ҈y¿æŽzí(8¿í-½R†`¿ÖNï|O0ëUNASNone3FGL J1514.8+4446?ï?,&™t?"ôa¦ÜD?˜{,у?"ôa¦ÜC?ïò­'Ñ?qO´Šè¼?Z¥Çï°_"?qO´Šè¼?ë®GÖ?«Öœ JS?ÁG²à§÷Š?«Öœ JT?ï—Îàÿ®?q-¶Ok"j?ŠGùÀb?q-¶Ok"i4FGL J1515.5-4242¿é¹''VÈý@)Zb˧2ßÀ:F;ÉÚªÀ;óò#žjº@€àîË¥@lè–Vîú?ĉûVxÍ?±Â2"ý¨?êVjÀh:|@üžîJI?Ҍùx&'K¿ål….¨‰÷¿ê@ý‹±yŠ¿âàÓ«¿è|ûhÁŠy¿Ö²#~4c_UNASNone?î™$!ìø?£Í‡Öö]?¦m¿Má0?£Í‡Öö]?ïj>.FÑ?¬³–Ïy²š?'¸:7-åÕ?¬³–Ïy²™?îv䲐AÒ?$4eç?¨'´ÖûâÙ?$4eç?ïFpëàV×?/xaµé*?—1âƒõ%?/xaµé*4FGL J1515.6-5817c?ëôQLt¿á̓ ٔ[À8éŠÆ—ÿfÀ:'Œri©è@àØÏ›y?ÿ›¨g'¶?ÎçŽD%ô±?ßϏ_Yø?õ,+l•T?ÿ –H+gã?íu'}ô!¥¿äXYÐUî¿ç›Wã¿ãâæIu"Ø¿î]%uŽÛ¿ïîÞoŒÖUNASNone ?ÜÞÀÂTqý?бâ"a?ᐟžÕÇ?бâ"a?ëÆ#T\|c?ÌT~*"Ô?Àçr®Žs?ÌT~*"Ó?ÚµOý	?´µýãŒ%Å?â¥|Ø~ü?´µýãŒ%Ä?ãT•õ%ÐH?º®aGõ)»?ÙVÔ´_r?º®aGõ)»4FGL J1516.1-6429¿íYoý\'ÀyԀö4¥À:Asqç£éÀ;¹ë\ÚÌj@c¢fǵ@ë'Ü5ö\?Ôvóý=Wú?Ù%ñaËØ@R$ZR[í@…ÉêoJ?ï×"ÆÔeH¿àÛ
bY'l¿è÷ïÅöö¿æû	 :2+¿ïþ,@OÑO¿îôÔ#&vUNASNone?﶐<JŒÑ?Û)`ž'?'[ðí\ËÇ?Û)`ž?íâ'0£,¤?¿þ1»Ã¶¢?°ëvzæšá?¿þ1»Ã¶¢?ë°æ'ð–?ª*(ûÏn?ý<e´=¨?ª*(ûÏn?ëËèWäÈi?¤&cIv	Z?ÀÐ^ lÞ[?¤&cIv	Z4FGL J1516.4-2640?퀠ȱ¶2@9âÀÆ.MÀ;':ûÀ='ÛSxM@¦¢Ç•«M?ÿŽêéîEÃ?Ù¦û¢"T>?ïx?ânÂ@
UûÐÆW@4:¤ì‰¿íŸXàÁÌ>¿ë5ݜþ¨è?ÖȾË,d¿×wß4®]v¿ïÿëþ@bF?Ú>‰¨ŠÎ%UNASNone?îvr…¦?®Á¡ÉwJ'?¨˜ß÷¥ž?®Á¡ÉwJ'?ì†Åoõي?ÇQaf\N?»ÉԀQ3¬?ÇQaf\M?覀'5?¶±Û)\ùc?ÏÅeý··)?¶±Û)\ùc?èƒÉØx+Ÿ?¹‹Åt¾?Íð؞Q"?¹‹Åt¾4FGL J1517.7-4446¿ÀÏ™Çðo@%w+#š8üÀ9Œ)s–БÀ;ÔÞ]	@³6	Qbs@ ò{²þÅ?»õÔ­ì·Ï?Á$HIDíp@hÚdeg@uó>#§¿Îú1^ò©«¿æp>Œ,ɍ¿ãï
¿[J)¿äÍLN+Í¿îM"¸aþ¿ï÷#M"MUNASNone3FGL J1517.6-4442?ém_l2åw?Â@‰;–
ƒ?ÊJ'O4j%?Â@‰;–
ƒ?瞇b…?Ð4pY7Él?ÑþÂñ:õË?Ð4pY7Él?êez‡Wr?±;[i'E?Æjâ¢7å?±;[i'E?é|aK縯?«¹x#QÔ?ÊzÐaF?«¹x#QÔ4FGL J1517.9-5233¿è÷ÔdØŽ@'Š^"3NÀ9….mє³À<
ÇÚÅ@…BüÔÒU?þpCÊZ+Æ?¾q)¸á—?ãssÊÒ÷‰@ —¨mqó@‡B¨œö?ïü'-ks?î"=ßßy"¿ÊͲûÀUE¿ãg¡yâÅ¿î—;»—ñ#¿íÇîÁ"4€UNASNone3FGL J1518.2-5232?W3ր½y‹?[NV—ÿ†?ïôf¿¡D?[NV—ÿ†?{Òùö‰æ?¡íÓh—%O?ïÈZíî?¡íÓh—%O?Œòò"«ùD?,›?âõ=?ïŒ45±P?,›?âõA?KqXdµä?:ö;mܧy?ïù#©þ¦Ó?:ö;mܧx4FGL J1519.7+6727¿ëISnŒ@EòxžwNìÀ;5Ñü·v#À<ùm"X9@ $©iuÍ?üGÐ^QÄï?ÌJ?(ßÈ'?ϵшžI­@l6|"ÏU@t§^ÿò?ï˱^²<ÿ¿îz´0ô"'?ÁXée´º²¿×¾Nî÷ð¿éJO^âäf¿ãׅøÒåUNASNone?ïܧ€Â§#?mÌK¶FSŸ?q¬?ž¬n"?mÌK¶FS¢?ïðáO5n?ts"7#§°?^=ça•$Œ?ts"7#§±?lÌ)?™ê%,'?¦&™3?Ým?™ê%,'?î8ö±´¥?'Àóh&‰?¬p"串?'Àóh&Š4FGL J1520.9-3805?²H±i@/÷ûH
ZÍÀ:}ke©¨À<#d"@‹ãJ<º@݊ú`"?¼+ö}ö%?°³'i#°?ñùYˆ1'I@¬ø¢¾†c?ïÿ™¾, ó¿à]d"Õ»¿é¿VŒÔ9¿âðP•CɃ¿à^Æz£4¿é9†3‹GÇUNASNone?ïîíœUÕ?`Ô;›#º?acªê+?`Ô;›#¹?ï÷vÒÂËD?i‡-éÔ#m?QZziw?i‡-éÔ#n?ï®$Í#°?"qÀX·¼¹?"vÌ·?Í?"qÀX·¼·?ï²·Å©Ôb?l?™cµÄA?ƒR•ŠçD?l?™cµÄ?4FGL J1521.5-8057c?ãåƒ2ÄÀ3Ö/'4ø/À: ÃÄæNÀ<€ãÀ.@ÜaHÅ@¼@cÃb(?μz-È?ÃÏeÙM¹œ?öɊ=D
@™ÎwFÞ?ïó¤r:¯ÿ¿è</áoA¿èm`áAMþ¿ÖV¨ƒAh€¿ð?ï÷vG…UNASNone ?ïô­A¿°?^–`Tw?V¥}րŸ¸?^–`Tx?ï}Uqî­á?¡€Æqgsë?UQÂ*CÜ?¡€Æqgsë?îÖÙc‡Âe?–O¥xNí?¢'iǃ٦?–O¥xNè?ïH"¾Eq?ˆº
èÒdÐ?–íh>QÛ?ˆº
èÒdÑ4FGL J1525.7+1503¿îIŽ@JOKD¢À:€øõJÀ<NúìšÈn@$¿÷t@öڜ™(?ʀµ^å?´C_Bå?çváfÃ.@V'Ìx"¿à'âLÒ¿êp'_ÀYø¿æ܀w¿ïÿ»6¢S|¿çlÊcfæ?ì A¾ç0üUNASNone?ïÿ˝Ȧ?~÷
Ú>ú1q›­ø?~÷
£?ïõ׀»s?~+S¶Û(~?TPÿ̉Ö?~+S¶Û({?ï¾9ÒëT?ƒ‡1—©³&?€q¿‹E+?ƒ‡1—©³&?ïô	³m"þ?Qb÷³"ŧ?Wì™$ö¬?Qb÷³"Ŭ4FGL J1526.3-4501¿îÁZ ;¶z@#XO	RÀ9äù8¶À;óé Àiè@;öófêp@ƦºêL:?¶z;°ZPY¿Œ•¢­Ù0w?ÕÁÔKFOp@'XŽó£?瘝N(ÿ¿åÁéå‡ó¿äâm©PÇ¿âø£JƒÄ¿â":‡»JÄ¿Îi{CÃ#VUNASNone3FGL J1526.3-4505?>£?|º¥¹Ð_?ˆ[pW;?o?|º¥¹Ð_?ïà"nÅj?«Z€*d‡?o{ã':"á?«Z€*d‡?ïc›g'FN?u"êô^?"Œ"·6F?u"êô\?ïsaEß^ò?zõG9:$,?'"×D!¨?zõG9:$,4FGL J1526.6-3810?éÐԞÝnF@.Ž­=%$À:ŝ%Ü3À<°ùïDÆÙ@ÊI±Nìø@l ºŠ«?Ê0pÍ¥»?å}¦‰l$ì@‰¡vݬï@-hŸ¦£î?ïÕ'^éšc¿â鏰â‹{?½Á]'çüS¿æ[Ûâ¿¿êíò·B!
¿ïæfÁ«¨UNASNone3FGL J1527.0-3804?´V—ÆŽqû?´‰w¬ûiz?íu-.1Á?´‰w¬ûiz?©Žè•ÿÁ–?½
Ë"ø?îgv æ?½
Ë"ø?ºq˜2OP%?¦Šdà#˜?ì±Ìù¶ü?¦Šdà#™?³Î9ìù"w?¼eäF[Ý?í†8Â`Ír?¼eäF[Ü4FGL J1526.6-2743?ãH(z̙@7®8ûÊZÀ:³*¸:n'À<¥Ãiv¼@Mâÿi,>@mæh3?̎BM'iÒ?ìq='‡­@ó'ªi@éR ‹Ñ/¿ß´[ÜõŽã¿Üυ
ñZ¿ÆGçà¤p¿äšyޓHÈ¿ïÿÞý¦ßR¿ç#î¢	ª¤UNASNone?‹½&|s?n¼´)¼'?—f?n¼´)¼?•G*‡sÜ ?¥Š1ï­˜?ïUÆ«Äa?¥Š1ï­˜?©Ë²òp©'?•™ôÌŽr?îcDÐØõf?•™ôÌŽo?•ûz'¸¦R?}éH—Žé?ïP$.Â:Í?}éH—Žé4FGL J1527.3-3103?Úü4ìk`@4ñá~4¹EÀ:åJrÀ<%1ðÃ@ú"\ñrŸ@Õ7ªÉ?Á·]ú²
Y¿"ÝLÌ·S>?Ô »¡×+@t³Pw¿ãÓÇÝúœ"¿ÐùW¥ƒh¿ìUŒŸ
FÖ¿á­IÿþR¿×Ōf«/ĿٙޣcòÄUNASNone?ï"?*ùÒ9?Ã鿨÷?Šð5A‹q¿?Ã鿨÷?ïýþÃs?Jó
+"Wâ?0ñç<nŽ?Jó
+"Wô?ïm,kÄ­æ?Ž›H½F?'Zr‡jC=?Ž›H½C?ïô¶ü'¬?FNO§ì?V'ܧÈà?FNO§ß4FGL J1527.8+1013¿ïdóhA[@HÁ´xB0ýÀ:께Çâ'À=ÏZ@Ѧ¦G}@dGšÉD'?ËãŸ6¼£?ïþå-7@''¡.¹Q@ÏUï˪c?ïöW	ÒÙ¿âô8ñ
¿¾Ôw»ù?ò¿êõ°»õ4¿ïþÈÈ[N¿íº(ðºßUNASNone?Èřýõ])?Æjˆvæ€7?éΙ€'¨¶?Æjˆvæ€7?¯îՓx`?ÃÍhq¹«?î"¦Èz?ÃÍhq¹«?Å 7¼Ž@¤?­E:"ÌU¹?ê—òÜo×?­E:"ÌU¹?'ÐÕ!Ž:'?€ì(£s†?ïiyVóŽ/?€ì(£s†4FGL J1527.9-4943?íAÿ©Ë–~@š¬"¢ºÀ:N õCÀ;‰Ö,Çß'@"zvž˜@öuÂú»ó?Ϝâ#v&Î?Õ§IEbø@†NÜ%´@£E9›N?ïÿèã«6¿ë3!à¥q¿¿ç·€4mÆ¿å9ÞHT¿ïý6âjBê?Õ
‹ÄCç6UNASNone?í\ÊvOø˜?¸†4ôˆ?µ¬M€;F?¸†4ôˆ?æíDƦ)?Ў)ðX?Ò%vr³Á¯?Ў)ðX?┑i¡Á1?·v>"Àà?ÚÖÝ,¼}ž?·v>"Àà?ç­zÖÝåe?³¤šÒdÖ?Ð¥
RD55?³¤šÒdÖ4FGL J1528.4+2004?áD¸/Lw@J¿
=p£×À;møDøÀ<"ìˆ3@@ $¼ev|^@¢€…Ì];?Å«®o´¿¯ûÄÃ$=³?çžQYŽç@#+¿÷Q[?í¨)µ/ë¿î±
õ´M?œÄ1%oƒÏ¿ß¸ªŠ¿ãbr†/YŠ¿Ø#lÁŸG.UNASNone?ïï+Å=?YÇÜ©¾?`Ôÿ:Âüæ?YÇÜ©¾?ïûéGšxE?[õ5TŒ½?@Zá–ìŠ?[õ5TŒ¿?ïÛÕyvuß?{øO²sG}?rCDÅ\?{øO²sG|?ïљš+J£?d$©K"ò?w32êZ®(?d$©K"ò4FGL J1529.4-6027?æ>l'LJÀ
ª'†VƶÀ:wP™u‡À;+;íìØ@cN€ÌC@yDàá6?Ì0_ïÉ|?â)ñk@«ýq°F"@ü¦
›I?ë–åõ'¾´?ä	Ñ¥y¡­¿åœ,ñВT¿éËÕ¡1¾i¿ëîjáö)½¿ï#ˆÕü÷UNASNone?—Èà#±¢?±å¤1G³?ïA¸û†âs?±å¤1G³?ÔëqH'¸?ÒÜr"<R7?åðŠG[¶¤?ÒÜr"<R7?¿i®Ë)½¢?¬RÛзç\?ìÊ&šÈL?¬RÛзç[?ÄÅóL}?¦¼ÆõóÂG?êθÃ,Ûá?¦¼ÆõóÂG4FGL J1530.0-1522¿Øù8l
@@V¤"‰—ÄÀ:°úìšÈnÀ<Ò¦*¡"@ÎÝÉl@žnëp&?˳+;-C?ãõÄ<ÛS@¶'ö @0W`¹ÿ?ïžæu¿±'	/(·"¿Þò¢¿æX~FVüf¿ïÿÿ&¦³?ïYÌ?SŒUNASNone?·|ÛÉýô{?º8…ïò?íd†ÀAq?º8…ïò?¹Ú<ÎdJ?àɷ'Ȭ?ìÝD¸f3w?àɷ'Ȭ?»–®jì.ç?©-±[xÖ¹?ì*2¢z#?©-±[xÖ¹?ÂÁG-ÛvS?°\"ÀI}'?ëO®4‰"l?°\"ÀI}'4FGL J1530.5+5850?ànˍc@H
r!…‹ÆÀ;0mWoÈÀ<­
‡¶B@´×xÍFD@b??°ï÷?ÄzIÚÕ¿¨ï¥È /?à>¥ÂœÈ"@çòiÇ¿â"±?¨Œ|¿çº=³¿µ¿ék¥^¿ÿ¿Û"à?¿ïüc]j	?ïŒËà"©UNASNone?ïê3 \¼Ü?g¾ˆ/6…ç?eÌߣC#¸?g¾ˆ/6…ã?ïÞG1êc?Æ÷¤Á?pò\g
Î
?Æ÷¤Â?ï¼?'ω?{jíhaš	?€ðŒ8Ý?{jíhaš	?ïæñ̏è?_ ¬fØrª?i<spå?_ ¬fØr­4FGL J1531.6+0406¿íËñ]-1x@F³åBåWÞÀ;VÔ"+¤À<‹Øž'&ß@
8=3<@Èáž)?ÎFacGM?ÃŒ¨šhw?öFl{S]u@W‡§£?ߪ_d"(?ïñgìxc¿¿çeà"œ¿ÜâÅB>ê¿ãžzߚ.ë¿ïÿÀ?ЀUNASNone?ïñà=
á¨?[ÕaÝa?\?…ê<®Ç?[ÕaÝd?ïùã3ò¾#?dՁ®¡
X?Hs05tª?dՁ®¡
Y?ïÌ!².'‹?yóE©XB?yï&è¾¹ð?yóE©XE?ï)ÓE?zþŒ?Ԙ?Œ¸õ˜‹.á?zþŒ?ԗ4FGL J1532.3-3857?ÞÞ4¹$@+ù"pŠ¬—À:Ò«>݋aÀ</"Bð?™@عó¬4§@Iß9¶Úó?ʽ	¶74?°"ŽJ[?çÉ[ÉTrH?üùä]K?ïø¯^|ã¿är5<!ï>¿æBµâz‰¿â^06ÿpŽ¿å'Ë9NÖ'¿ï×G²JkUNASNone?ïï |ÈÈ?aYõa‡B8?`ê߃78Í?aYõa‡B;?îáCáI€?µŸèþ±®o?¡ëÁëgþ(?µŸèþ±®n?ï¦ÚïB¡…?'öú¹:®?†ID/Wžª?'öú¹:©?|."?Š+'¿\ù°?¦h>ͺ?Š+'¿\ù°4FGL J1532.9-0313?Çq¡{̯ô@DR)AAé¯À;Z4ù»À<ʽé:ø@4ê˜d»@¢®Ñ9C?ÖTéf`‡)?ë6ˆ™"º@	 &5@H8}õÏ?ïå²af¢K¿å±ÏñD{Z?Ók—}µk¿ç¹¾!ä+c¿ïÿ¿h`;ª¿¸_ô‡PíUNASNone?èýc´û€y?Ä«‹tcÀ?Ì
q,þ?Ä«‹tcÀ?ÝA3¯£ø?ÕG3·¼]K?árßf(.?ÕG3·¼]K?åÀ›M.V?¹)»jÑR¡?Ô~Ée£éS?¹)»jÑR¡?ÊÚsvërõ?³ÿTÕP¿º?éIc"E#D?³ÿTÕP¿º4FGL J1533.0-6239?ïÈ­ø"ËæÀ†¯f•À:w
)´.pÀ;¬;Oag#@ȯ+|/¦@È˛te-?ÛÜ:¾lâ¬?í:û@
þ
A¢a¿?þì¸"ÁE?ïâ, GÑ¿Ód~d‰íT¿ì&½F¿êÍì‡}7c¿ïÿØ]#Dž?ëÛu<Z#UNASNone?íY¸ëÞm?¿ïî
ˆÔ?µ2?ˆ¡ ?¿ïî
ˆÓ?à|§6͔!?×,öwk*%?ß±'d×¼?×,öwk*%?ߌÒ1¨I?·øԆƚp?à9–çt«Ü?·øԆƚo?¦då¯0=?œzô_RØ?¡¥ü?œzô_RØ4FGL J1534.0-5232?í"íº™n@QÔ=ÚV"À9—$tSÀ;NѼÖ_@¨a3÷~Q@f":Ì?½-ݳÏи?͛ƅ
ƒ@P +"?ø±\"±*¿î	\Ý°Ë?ïûPÙ6g›¿âÛÏ3¯Yõ¿ãðV+Ü¿èÏ}¶åû¿ê'úhçJ'UNASNone3FGL J1533.8-5231?²,ʬéAh?³TKž·1?íºfªb×Ó?³TKž·1?³c4üŽþß?Âdb¤ÿ]L?퓙`n $?Âdb¤ÿ]L?Õ5úeê?´XÛàW³W?åreÍ
þ?´XÛàW³W?¾}î#…Ç?¨œÕÐyß?ì0B;H?¨œÕÐyß4FGL J1534.3-3312?Ó꜍¹O]@2WÙÛ©¢À:ßØy©9JÀ<~Ú©.b@‡‰6õàl?ýL¹ñ'ö?Ñ»è#'?Ýp¥°@
E^³¾@oµ9Þ,?í`L•ÚȿڅKCuJ°¿Ö…ÜãÆ8‰¿Ú'}keª¿í²Ûe¿ïñn7@UNASNone?í02­®–…?³@§©y?¶~j'‹KÚ?³@§©y?ìÅ@û.í?Æ9[p§ä?¹Õø&ˆ—ç?Æ9[p§ä?ãÉú«©†?¾³Òç‰*à?Øl
©è¬ô?¾³Òç‰*ß?êlì	—‡?¦!DÖXk?ÆLOÛ½¡ã?¦!DÖXk4FGL J1534.4-6719¿íeE«êßÀ"ÞøH{šÀ:ª'ݽµÙÀ<9v+ÖG @zJ''?@(:6?ÎRçÃô*?ÒqÁä;~[@m^!ôFŽ?ù´à‡iÁ:?ïæ†è¼í?ëP›ÄDæ¿Ù?""Æ¿äHcUeb¿ïük 	ŠÃ¿ïÿÄ;-ÓxUNASNone?ì´éµ;?¹OÁ£×H?¹ê_¸²V!?¹OÁ£×H?àèî†Ëõ"?ÓÓªëw2£?Þ."òhÙ?ÓÓªëw2£?ç·->ñ¦?±iŽ¥;¼?Бõ¥'´?±iŽ¥;¼?Ïö2UÔi?³@Uj£å?è9'sjŠå?³@Uj£å4FGL J1534.7-5842¿æ'ÚÏ`e6ÀRzÊÒÀ:¡s¥ê	ôÀ<–:º1¦@ 9ʆÌbo?þð– ÀÕH?Ò)0æQÙ?ïþ©Þá!n@kpüÂ]Þ?úô?Z2üW?îôÁrüvß¿è
þraF¿Ôsíw¿Ð¹PC9e§¿í²UB&Á
¿Úk ÀÀUNASNone?Ñ¢}ïߘ÷?̅
^^°?ç.Á3…?̅
^^°?À·âoÏV?Ën¶º³?ëÒ|d+?Ën¶º³?ÐSyÇásT?¹ú	SGµ¿?çÖCFV?¹ú	SGµ¿?:Añø†_?}õ5áïš?ïƒø8æ?}õ5áï›4FGL J1535.9+3743¿ã\1Æv%@KNã'áïÀ9瑳ò
tÀ<"âɎSë@–íÐÓl¤@™Ãیƒ1?µ
A\Õ?ÉiÊßaÏÔ@Ï8ÅCk@ǯPY?ïjøœ^oø¿âûµþ!s¿âOX}o—h¿ê«³AáKà¿çv"|#g
¿äk_ý–™UNASNone?ï€Ρ'\?ƒ¬~8Ì?úWŸhã?ƒ¬~8Ì?ï÷â_gì/?dõ
'~Gn?P;A0'¡ý?dõ
'~Gj?ìþJLy"?§»8NË®?¿X
­œ6ô?§»8NË®?ïÏV'±ü?dý_wâ¹?xT¶§¿z?dý_wâ¹4FGL J1536.0-2729¿îƉ"6[È@6"9:´0õÀ:×ÌQ|ÊVÀ<I"G!þ@dš½."@¿]þ¸Ø#?ȑ²ZÙ.?©󼥸6?âȕз=@rƒ.H<Û¿á#bp7 €?ëì²ÍOÔ¿éj¡3–Û¿Õ6—;~Ü¿ëé[x̚x?'E¿&ñÜQUNASNone?ïºÑ§3i?ƒ©¡á!?K–39¥™?ƒ©¡á"?ïû'Ü$é?_•ÉÏy¿L?A»ÜlXa?_•ÉÏy¿N?äùî?Š"'Ò?Üø†Á"s?Š"'Ò?ïÕUüx~?f`%e`_?uUÃüA?f`%e``4FGL J1536.8-4327?â¼#±1yÅ@#·ÃøôõÀ9­‹0JJ§À;¨#ÃS§G@¬º†¤ƒ@™åóí?ǵrþzCé?Ó4# Ál@€IÄo0:@/¡¨Ü­•?ï¸\Ó?­•¿ãšµùK°Ø¿ìpgÁ°9¿à™¬cû¿ïÿ݀y7$?ê|'œýÒ(UNASNone?îÐSú+V'?©q#œÅU¤?¢úÀ]JŽ?©q#œÅU¤?åV9!ƒœ?Ó$³[Þô?ÕS¼ùÊÈ?Ó$³[Þô?êír~'	?­P&¨½¡O?ǀJ6·Û?­P&¨½¡P?êôí"
Œ?°9RþY»µ?Ä,IïË©Ñ?°9RþY»µ4FGL J1537.3-6110?Ù
^h&üœÀåë`5ʽÀ:¼înÞ-À<5ÈÝT@9ג"­@N:Wê£?Ô#";9?æþ
·x§²@)@þÍÐÙ?ú¸6OL,?ïýi¸*~Y¿æ>
ÝS­§¿Øðh]a…¿èWJ*,¤¿îÓ6=ª¿ïȀâ¾|UNASNone?ÚӛE!?Ï¡ŠÌ¹Åõ?â–2r]7ð?Ï¡ŠÌ¹Åõ?ÖéõQÀ<!?Ô÷5Às‹?ä‹Wáð?Ô÷5Às‹?Ñ Äîsã?·Ïl´ÇZ»?ç/ˆþF?·Ïl´ÇZ»?­ hœ±Ä?"Ù¾ *.?î-ùv4ï3?"Ù¾ *.4FGL J1538.0-4638¿ìÉGÞõÕw@´À>IëÀ9¥£×àýÀ;V$fÖ@Mj¾È5@k#Â|ç²?ÄK9?ØÆÝ"/€@͌ƒ"_?÷΅Sç]È?ï"ßµ§í¿ärEb	àT¿æœ­äª9¿êðz¼^À€¿ïù¡¬'$¿ïïæ­H£UNASNone3FGL J1538.4-4656?Àéyá(?ƏÈgR-b?ëÅ¡ºµú?ƏÈgR-b?©¡Í§³;?·C$î%Šõ?îeã%"ÌP?·C$î%Šõ?É&YP]"?°›€À…?éº6i«èœ?°›€À…?')á¯|?kÞ@Ÿ~?ï·X{±C'?kÞ@Ÿ~4FGL J1538.2-6201?焻žƒyÀåKþSýÀ:%™kvqÀ;&hI•u@dð9äRP@˜ þ?҆¨%M—c?ц^~e‹ ?úoŠfö¯?û:+õÒ*¿Õ<â^"o¼?ï£éIUпêoÞµ,¿çÒñ©ûçm¿é"µÏZEÇ¿ïó!ž¶9UNASNone?æhùãE??͘™â_á–?Ó.9u?͘™â_á•?êPÖßÒ?Ícb/iÃ?Æ¿³à¤€¸?Ícb/iÃ?áÐVî8£?·Xg•Y¶-?Ü_Sô#Žº?·Xg•Y¶-?ÝWれm?ºtû'Æ}"?áTvŽ>¹É?ºtû'Æ}"4FGL J1538.9+0425¿À)ɾČa@F
;:iÀ:Àß}©yÀ<dQüLY@E…x2Â@äG<Õs?Æ1'®ñp?·ßj‰5É?ððhGçö@(U+«u¿ïá) ¸FÙ?ïÓô©Š¨e¿àò¿¥œÝ¿êqðdx¿ÐgÔ$¯â±¿ïùÕ^kÆ"UNASNone?ï܈èèÞ7?sE¹ãDWœ?q»‹‹äi?sE¹ãDW?ïøÀÓԐ?k@Tnš4ò?Lü°­¿å)?k@Tnš4ô?îô˜Aþj?•Áé'àJq? ¶{æ R?•Áé'àJp?ï•ûFÛ£?|F6ÔLÏö?Š¾A.IA?|F6ÔLÏø4FGL J1539.1+1008?á3"ä@YG@G†Ð'}kfÀ:Ÿ9&A³À<WÛçl@3¡B/z@ÙÓËď?Å5 ÝD?±M…C÷&?èh¦è6µŸ?õËÂƹU?ïÿéà
v¿æùÕ
ãîR¿ëË>øcSŒ¿Ø7ÑþdõM¿çdßI® ¿ïÿæŸÜ©ºUNASNone?ïòRÀÿŸ?i'WOÙ}?[Z~ØÃ?i'WOÙ|?íÜiu½xZ?»µ‰îSP6?±´R=.?»µ‰îSP6?ï€×—o?–ÿ\ u¾ð?ŸoåmI?–ÿ\ u¾ñ?ëëy4¾|?¬Î—IkG?ÀR/‰?¬Î—IkG4FGL J1539.4-3323?ì'Tò‹@1ˆ5ĊßÀ9(¼QT†jÀ<süQ×@ô$ª"N?øÿ0F祥?´þï3Ôî¯?ä']<ñøÖ@+‡_•'Í@æCÍ_CÝ¿ÓVºÂG¹?ïùgÁf?¾"–}/€¡¿ß';#l–¬¿íH>]2àþ¿ïéŸ
ç»UNASNone3FGL J1539.2-3324?`¥ÿ+OÕ?_a$œT¨?ïïZåÔ°?_a$œT¨?gÙûÙEx?v¢É¬jœ?ïè&&ôº?v¢É¬jœ?ºVñ½?§~2bcò?ì¿°!É?§~2bcò>âÝOËÍ>ßÎR àÐo?ïÿíã"°5>ßÎR àÐo4FGL J1541.2-5201?湫–³‰}@rkݞ¬(À:×t¼j~úÀ<"K<¤@"QÂ$}@o$ù´Œ?Ög½ž±†u?ïÿV¢N@
ï×hE@ÀUE+Ù"?ïñ¦ ¿ç¿ì3	ý¯Ã¨¿À'åbšÔØ¿áäñ`®—¿î0¡™¹¿ÏèŸ{°ÐmUNASNone?ãEÁâýq?˔–.o8¢?ÙuÀ|:?˔–.o8¢?ͯÔ÷"E©?Óg%!Õ0?è"
Âî–?Óg%!Õ0?àY\²?½!ë‰CÖ?ßMáGûޝ?½!ë‰CÖ?Ãbѧ7ÄP?°[ànA?ë'K–2ì?°[ànA4FGL J1542.1-5901¿ïZ¤˜6wZÀÙÖ»cýÀ9H.Ä8©•À:èºÃµÌÖ@…‡°@ìJÆͯK?Äwøõt¶¶?ÂXȃ'ðX?þcˆÕü÷?û")ÿ°z¿à¢R‡"Ä?ïÿRü&V¬¿æÆ×Tæb¿ë®\Ÿ=H¿îÏp;Ñg?ÝßNdgÌUNASNone3FGL J1542.4-5911?é57"¨»?Æ]²*>¥é?Ë£+!í]?Æ]²*>¥é?æšG
åê¤?ҍ&*ºŒŽ?ÒËqä4*¶?ҍ&*ºŒŽ?äÒn ¾Fþ?·$—5C…?Ö[#¾ƒr?·$—5C…?Òxˆ
YÜ4?¼¼ ¯ãV?æûúÓæ?¼¼ ¯ãV4FGL J1543.1+4209?¹N÷¬ðí~@J1a¡Û‡À;s¤ÎóÀ<ݜûMé˜@ .ÝNûÖ?ý¼\!iT?Ïíþ÷ÂD?ÌqG€r+A?ý™s,Û@	¸vk5X¿åõí!Öê]?í¦¡‡N¾?çV)Ø@ž¿ãh³¦Äz¿Ú®ÏÁsÓ6¿äÁœýýtUNASNone?ïø½"Ûª??NÇj_å˜?M	°'WÅ?NÇj_å?ïü‹½\þ]?T¡¹½ÝN?;¢
ó?T¡¹½ÝJ?ï{ozڜ?Šv6MÈ?Ÿò¤¬³?Šv6MÈ?ïî—†¤B?Q^òÒS?ahüy[¿?Q^òÒU4FGL J1543.4-5925¿îx(]eP}À3ý»'!®À:žlwø_"À;°ñ~\ý1@hwê@$9Ãp,¹?ß#v\}¯X?æQ­Dq@•%t-Ï?ûÍ%7G?ïùrz(¿íUâ_±?€ó;#Ë¿ãéošÂŽ…¿ïýn?΢¿Ý
v[Q	ˆUNASNone?åtçԖô?ÏtyduT?Õù0VÒ?ÏtyduT?áNbóò?Õ½^"‡ß?Üßc:ã?Õ½^"‡ß?Üh¶ÍIùö?½º•_râå?áˤ™[?½º•_râå?Çò3F	Äü?²Îu2B§c?ês.}ŽÂ?²Îu2B§c4FGL J1543.6-0244¿âªÄãÓrX@Cqà?pXÀ9òµ™ªaÀ<(P!Ô@$o¹Ì?@¥zxl"?ÂCK¯*ûV?Ûè]»Vƒ@`ûH
?önrtÈû¿á¤þ§R?ێÆ!7S¿áâP>ܵ¿éšïª/>¿î±±RóÂÛ¿ïÿ"	¶UNASNone3FGL J1543.5-0244?qGÕ>1B?yq(ÖgF¶?ïÝpUƒóž?yq(ÖgF·?™'²%³?¡Ôž;IÁë?ï3jnӒ?¡Ôž;IÁì?£âAªm(?—¢2)‰S´?î΁ÛåY-?—¢2)‰Sµ?ƒÐ£­NàM?nk]ëš?ï°½qJÄ?nk]ë™4FGL J1544.2-2554?åã)Җð2@6š€JœÜÀ9žµŒ>gDÀ<n5gÀÙ@"áÊà¹i@ÁµQà?»ï¨ïÍÙ?Øçz"0¤@ëOKD¢@Çÿ_¿ÛÒæÂAX¿Ô³7¥]È¿à`W=Ôvå¿è½¢B4­Ý¿íEK-û»Î¿ðUNASNone3FGL J1544.1-2555?'q Ž±Z¬?³=²R•2?ïtvûŠu+?³=²R•2?'|4ü¼R?žqJk`3?ïlXp?žqJk`2?"ħðâjÃ?1ï0Ö¥t?ïYÚÀxìª?1ï0Ö¥y?®ïCÚ+?–xí˜?îKÂ^<?–xí™4FGL J1544.9+3218?҇ŒÊÌ3@JÖÜGªÀ;Am
ÅUàÀ<Ç+w}@ ʛþ"Û!@%¸Që…?ÀˆÔº××ÿ³,†›»ý?ñ4XÖZë@ìU¿û??ïÿ?{@?¿íRŠ±ŸIÝ¿×M,Ù|Þ¿ßÖïEG²Ç¿Ê±"øu7¿æÒÎ8ݗUNASNone?ïüîބþ?48Vœâáx?8‰ÛxÇ?48Vœâá'?ïüD£L¬ø?T®ýœh"0?=Ú嚘Dç?T®ýœh".?ïð3!zƒo?i'`dËêY?_™½
ù!›?i'`dËêZ?ïÕãä}‰®?c~‰X°?u
Á;(š?c~‰X®4FGL J1545.2-4553?Ô¤³ãD^@O¿ZôBÀ9òóĈ[À;{<¤ËüÃ@U}£ôC@‹Äߘl?È9…‡¾Ð¶?Ԓ±êˆ@	¹JÚåª?ö³:9·±³?ï½!~TÛgå!I¿çši£1Èпå³À¶‰?¿ïþñ­VåÀ¿ïÔ'£]éUNASNone?Ñ&ϑ'¾Ë?Ç~›ÏeàÛ?çl˜77 š?Ç~›ÏeàÛ?Ì]›@ð"L?ÏxáélÓ?èè™/ÃÞî?ÏxáélÒ?Ó¤M«{õ?µ6üS²Ô­?æ-Ù*By?µ6üS²Ô¬?Ÿò½2r†?ƒU¬GI©(?ïjlk"?ƒU¬GI©(4FGL J1545.5+2839¿¾G9{Â@IÜ1&éxÕÀ<£3vOÀ=Ñö®H@¾d`QÏV@ª×DÁ?ÙfÀ=ó*°?ïÿøÞ£Žæ@
š;e0ÜA@®ˆ7q†U?иw?Ò}ç?ïÿÁeÖt?´Â9JúO¿ì†×6&-¿ïú™Ž±ß¿ïÿý±q&´UNASNone?ꊏ¯Ÿç'?Ë+OˆÏˆ?ÅÕÁA€a·?Ë+OˆÏˆ?ÖÛy7UZ?Õ=IØmpÈ?äô'CdUS?Õ=IØmpÈ?à\½ùY,?½ªT˜^èn?ßGЄ
M§?½ªT˜^èo?·³FŠz2§?¡O^n,å?í	—.°¹«?¡O^n,æ4FGL J1546.8-3244?×}´†™2>@1¢ß"xîÀ:ÀoB­úzÀ<m¿Ü#å@ r"õ@ÓðØï?€"º•Ë?«éÃþr`?ì8é‹It¾@+2ËÚ3"?²b× ôÓb?ïöѵ(k¿Û_9áÎÅ¿å¡Äÿú¢¿à¬Ô>±·¿ÚàÏ6iIUNASNone?ïøTËu«
?Jύ¿Ð\ã?N¬Ò)SÊá?Jύ¿Ð\÷?ïúýÿò?hÌóh Ä?D7£åb?hÌóh Ä?ïÒõAdÁÅ?y¦Ïn"Èê?v…_MŸÌ?y¦Ïn"Èì?ïÜ1{Í%€?_û¶GÛò?qçBm?ß?_û¶GÛò4FGL J1547.4-4802¿äÿëBŸÝb@o'½†,À9 MÞ°$ À;lÀh:{ý@+Ý~uÒ@ø1jWX?Ã=ÛØ®Wl?Ә•=×@äZÏYo?ÿlå#/Úä¿Ö#fmG¿á'u=™¾ƒ¿ç|OÁß3¿æN-Š|Æ$¿ïþè=k›Z¿ÀsiN¿UNASNone?¿ì%0yâ?»uW1¡G?ì~{YðÄ?»uW1¡G?·@³%a²?¿_‰Q‡ª†?íé›SßÉ?¿_‰Q‡ª…?Í}jg›?²&W$??è ¸þ%f?²&W$??ǛG86b?¨å.™aÊ?ê.1ògy?¨å.™aÊ4FGL J1547.5-5130¿Ñê¡ûï]?@÷RØҕÀ9C»€t.¦À:æ]	A@»¤"ÈŸA@ãO%AI?À8›Ñr?uကFv?¾=îß,‡?þ"jCk?ïþ•1U¢¿åX5`´ö—¿ë	¯Á¤$¸¿ÛŒ\å^>$¿ä8z?Œ1ý¿æ'zç&ë&UNASNone?P3J?¤›[uQ?¤GŠüË^¤?¤›[uQ?î6u{ë\;?Á5®¼:ø?¬˜¨AJ<H?Á5®¼:ù?íjôŠüO?¦WȶF?·t¨[¨…?¦WȶF?퐇æ¯lU?›i˜Ó'"€?³{ÀʄV?›i˜Ó'"€4FGL J1547.9+0445?íÛhýÏ;H@E5@N¤©À:ôéË
TîÀ<K¢î¬ñe@頚¿´`@½¶°_¯?Î˔¨î÷?{þì.¼Öà?¯ ^¶ï–?ýŒ Ãås?ïl….¨‰÷¿ÛÜŸBÑ¿á‹Çêüó¿á­.l$‰¿ä¢àj8'þ¿áB£þøCUNASNone?ïö	_eR?QßõÌñu?SçíA5\¬?QßõÌñp?ïîï•Zá?w³Íêžùc?aj¥ðî?w³Íêžùb?ïÈAPCÞ?~ŽÃ)ª}í?{ßWÞþ\?~ŽÃ)ª}é?ïxÄ%êCh?wæu4Ú-¤?ç{B·'×?wæu4Ú-¤4FGL J1548.1-4416?ïŠp1ºC@Þá"Å&æÀ:‡0áI\À;Ã?¼®q˜@ËT‹rj@å"Ùîô??ÈýGéΐF?á]ŸîGq@Mý&0ì1@)ÓøEÃ?ìr>
þ¿ã
n}Œ¿âÅ~ú±âf¿ê "Êý¿´¿ï÷2œ4~¿ï 0âvdUNASNone?£2í5kã?¤ž	0yäÙ?îÌ߁,©B?¤ž	0yäÙ?²lçÑ"—?¿©Œ=üí:?í²cÛ¾-?¿©Œ=üí:?·\ ê[Õü?¥ÓŸ?í{ⴅA?¥ÓŸ?¢:0Ó?‡'*P¹|ß?î×\ÿâÑ?‡'*P¹|ß4FGL J1548.3-2411?׸ߗmø¤@7DIDíoÛÀ:†Ôt`úíÀ;ú—t%kÊ@·É³å±@"º\‡À?ÒE3{W3?Ì
/Ä=Ý?øÌs@i|›@j£·Õš¿ìFX^»Í ?íªü-¨…¿ãçŠ$Óõ¿çP tοê%~>Ê@+¿ïû?ÏLÚUNASNone?鄮!©?{?Ä	B6þXn?ÉíGy[?Ä	B6þXn?ï~eT)¹m?£¹ögÊ)?3UzÈÒv?£¹ögÊ)?çŠEŨ˜?´uZ¿!?Ðëtt¯úÑ?´uZ¿!?í‰ë¬ÂYV?ÒIS—?³°¢™í5T?ÒIS™4FGL J1550.4-5354c?èU¿Y°z?ÌRó—罿À8}N€ÌCÀ9ú&	Ã@τ'Û9@ÊÄç%>?Ûqšânõ?Ì
>ðÛu@1bBë7@m%-O™?ïþ˜½?;?"¼ñ@'@¿èÇÚÄç%¿êë)CÆ(n¿àÞLÑë¿çÓÀì÷UNASNone<?Ò~°²\ð¡?Ð<Í6K/&?æÀ§¦Ñ‡°?Ð<Í6K/&?ÅçåÛ žo?Ì«èå?ꆉ7Ød?Ì«èå?Ñò_Yl7?¸×_¼#m?çÐÓIä?¸×_¼#m?ÊÄyÑÉ÷.?»b¬¸B?éNው'4?»b¬¸B4FGL J1550.6+6027?æÔJ/Ä©@F‰"_ôöÀ:é5WСnÀ<ÒÝnÛî@ q¿ºëxß@³Y¼3øU?»__(R/¿³è‡UYh?ôý7Σg@¡Ë:¦o¿çxÂ
?©¢í\M¿ç›8 Z}û¿ÊžI—"ÆÔ¿ádãD–Í¿Ú4Ci\UUNASNone3FGL J1550.4+6027?ïüï5ôK?5²ÇÌ£?8†P]§¨?5²ÇÌ£?ïý•5…?PuT¥Ía?7KVS×rJ?PuT¥Í`?ïõpe´S?h™ˆÔ/?U4ėY´?h™ˆÔ2?ïì›ÝJã¨?QßõæˆmÉ?cd"µWø?Qßõæˆm¿4FGL J1551.3-4920¿ë1ò_¢üý@
x¡Ú°»À9҃pbh«À;/Ÿ(NÓ£@s˜.4›¾@P¤þQª?Í×yär…Ù?ÁNÔäÉBÕ?ô…Őe?ûÍQ¤ãNÄ?ïøM·†ê¿Þ3LÉn¯¿êâѼÖ_¿âhá}V¿ïø¸BÒ¨?ïtã׫MUNASNone?î¸ÑÏZ'µ?«Ïʄ±Ü)?¤rã
WÔ±?«Ïʄ±Ü)?êÿúÝ?Í
ëL'3?ÄÈ‹è‰?Í
ëL'4?êEh¦Ìƒ?°yûwz°?Æê]dÍóó?°yûwz°?éêgƒè?³,Ý}XðÔ?ÈW¢að_é?³,Ý}XðÕ4FGL J1551.7-4257?§ÅÊÀ÷¯™@!*2	g‡ÏÀ9ԗt%kÊÀ;‹Ûz¹×@ššÊA¥@Úú—
s?Ãóâû¸G°?¸¹Š¿zîx?ô,byqÛå@ªëhÄ9«¿è4ÛϲZ¿áâ~
ÇÚ¿éGimO¿åÕ¥¹b¿å"&"À¿ïÿÀ	oëJUNASNone?ïÉëž"ø?€i×86Í?{
0ÿ=ƒú?€i×86Ï?ïU—jG†?­îC'"–u?•^-·G?­îC'"–u?îEÆÑ{ž	? K?y.B<?«£'èFm? K?y.B<?ï1ÞÝòÒ1?"‹°Õk?™Ä$A¥¹Ï?"‹°Õk4FGL J1551.9-6015¿ïÿZ¬Gk¨ÀYÓpóˆÀ:lù¹"á¤À<
øç
¶@š>C\¡@÷ÀOæÈ?ÔðÍÝîÞ?ïÿÿÃw@zæ ³iN@Þȇî¡^?ïôž"|å?Æö©j(€¿éo`
+Òí¿ïôQ«Ä>‰?é©£½^ð¦¿íMt']è¾UNASNone?æÙX}ƒ'?ÍìùljÍÁ?ÒMOöøÝ?ÍìùljÍÁ?ådˆbºqå?֚Æ?!d?Õ6ï:‹5?֚Æ?!c?à™>i"úâ?½œ¥f¨?Þ̓,Ö
;?½œ¥f¨?ߛq9ëë\?ј7¦&•Ë?à2Gc

R?ј7¦&•Ë4FGL J1553.8-5325e?ō¤¨ë?Ñ×r"eÀ6ˆËà=ÂÙÀ9‡‰Fe?@i9È£T@EüÁ‡m?ŸÊ
ª¸?»Q†'_8@¢l] l‡@©Ç "?ïÿÑa\w¿É_·
BÏ¿à-â@ÒX'¿âl"þª?"¿äžJÞÿâ-iànjAUNASNone3FGL J1554.4-5315c?ǂ]60î>?Èy®ÎÈþ?êh²sÄq?Èy®ÎÈþ?€ËQ¨wQ4?¡ªyqªêN?ï¼Ò¹^"»?¡ªyqªêN?䮆7ãJ?¶,^<L3(?Ö¢óŐ9m?¶,^<L3'?e} ÙöÚ?UÛFsÖ¾~?ïê'è_&	?UÛFsÖ¾}4FGL J1554.2+2008¿áÿ/Õ#Ä@Gäñ<îØÀ:³È±µRÀ<x úK‹@!x?×±W?ûQ¦&oÖ?ÁÆ£}sY?·KWí&ßh?÷zÀûÞ2P@I*-¦…¿ïÙ	Y¿ï@…3Ç-?ïùV˜"	]¿Õ\…ýZ‰8¿è•övêB)?ΗådsGUNASNone3FGL J1554.4+2010?ïû#Ս%{?A,á6¾?Cp©Ëj)?A,á6Å?ïú&9F¬?g	ãÂ$Â{?Gg'åP'?g	ãÂ$Â~?ïÈ,!µ?Y†¬ó?{éï%|ý>?Y†¬ó?ï¥!Z"Àî?zߎï3?†·©ZÏĉ?zߎï24FGL J1555.2+7103?ÅÕL(Rÿ@Cš+<¼IÀ;
iŽÀ<å4W¡†@sgÇ9ï?þJÀ¾¡'?Òà!1H?ÞG^á™@h%ç}R?ý2xUQ@:¿ë64¥#:˜¿Ðô!:kH¿Þ¯_ÑvÖ¿åÑva†-¿ì´
(wîN¿ïüP}ÆÕ<UNASNone?d·¦?¢s0ê"YB?¤h©´…›?¢s0ê"YB?ë¨w%þ¨?ÇΫ30î?Á^#hÅd?ÇΫ30ï?èÜ֏4ß2?±5ìtï+?̌¥Ã,ƒ7?±5ìtï*?䆿}Ïi?³¤ÿaÄÆ?Öòa×,?³¤ÿaÄÅ4FGL J1556.4-6911¿å]¬RÂÑrÀ'öº «qÀ:¶"ÿ®¡iÀ<qzØ
r¯@28EìžN@ðüõŠ?ÏcæÄŗN?ÙÙØN
O@¦ÝA‰?üŒcXÊÇ?Õ%ðál—?ïâàj8'þ¿Þ•¨sQ0t¿Úf('íמ 'ñ¿Ô×[œãUNASNone?çÅ#^"df?Ū~°½H?Ðu¹BÙ73?Ū~°½G?âTëŠç˜?ÒA‰¿Ü-?ÛùV(ê0Ñ?ÒA‰¿Ü-?çVÆÃ5?´"Ûä~?ÑRry×Ø?´"Ûä~?Ùú+ñ`?´ZϒsÛl?ãêO÷þ?´ZϒsÛl4FGL J1556.8-5242c¿âú
·Wn?áG›*½™À8ÐÎ{ùu¢À:Qqâ›k@ž>õ3HW@ ~ÅؼÅ?ÍÅrûË
?ÖZÚÂïI@
Ødà
—?ü…¤DBz?ïó…hŠ-¿á{%oü^¿äÇ QºÞ¿éÓ¡Ó#ÿ¿ëTu£KÜ¿ïÝ{¦i‹µUNASNone=?²&£k˜3°?³Ëº~ )?í»+'Œù‰?³Ëº~ )?½}ßVq?ÈØø?ìP\|Ä2?ÈØø?Ðdöàf?¬Ð3­Ø1)?ë8[æÂGæ?¬Ð3­Ø1(?"Î:é¤í±?E7^v–Ø?ïYŽ(²Ø'?E7^v–Ø4FGL J1557.2+3822¿b[-Î7³A@HåæFñVÀ;ôÅjüZÀ=ž¬(—@ TÜY×`?ýZ&6Ën(?Ö6ë¤~O?ËÍ&#€7É?õ	:q@ÿxÍFD]?í :}Ti?Ô¢˜[V¿âå¹ÏD¿¹u‰€-+¿êÇøð?ŠÈ-UΓ¡UNASNone?ï€à4Z?‹¶±$Âé?Çà²éŒ?‹¶±$Âé?ïørfVh?jô^¯Sb?N6f¥Â[?jô^¯S^?îbº¯Sß?›"ì*#?©Ô^¥
Â?›"ì*#€?ï›Ì‹ï=?ucÖ'!i?‰Ý:D0o?ucÖ'!i4FGL J1559.7-4518?݆>ºÝ1@nžÂÎFJÀ9¡Ä©èœ6À;ULf
 @¬3*úª@°#¾…â?ŹxǑúi?ŜçAm2³@ÅáõRþ?ù¢¾Úzà¿ìZÓÍ$á¿Ïߒâ›@8¿åÕí¨§c¿æÈÙ"E¥¿ìEÞ,ñ{¿ïúÿ?8$UNASNone?â?'Dã?Ì\}˜¥(?Ûû€Ûv9ç?Ì\}˜¥(?âRìZ‹Ã?ÓI­X)a?ÛZ'JéÎz?ÓI­X)a?åsíI=?¹aÀo©*?Õñ%mû"?¹aÀo©*?Ýr÷ü´1ú?¶è"êW*õ?áF"¥ç?¶è"êW*õ4FGL J1600.4+0407¿Ôk=RӚ@C¸ƒBÙÀ;	ð€0<À<€Ü…§tN@rX¡×«£?ÿd¢¬gÒw?Ïe»d°?ÈPIÄo0:?ùꁘñÓí@+´Ýí±t¿í‰Ú¿~°Š?ïÿVW$ª¿Ëú|]s¤¿Ú—8Á< Å¿ïÿÇËÜ?ïýjŸ>XUNASNone?ïùŒØÊùƒ?M_«Œ¢Â¥?I̜ÔõF?M_«Œ¢Â²?ïùîÒ—ø?k9‡¥qö?HD·å  '?k9‡¥qù?îßhn\Œ
?•'¡ór¯?¢	y7?e?•'¡ór°?ï¼¼b#?tK'å{?€Ðú'w{?tK'å{4FGL J1602.0-4402¿ãÞ
yÛ@-Õ
ˆïþÀ9Ú|#g
UÀ;h¦Bˆ@§*ѺÈ@_tÝÛ?Ã|(ÚêœÁ?—Ì—ó§,)?Ùhm
&Ú@úã(-ñ€?ïÒ6™A¿áÂlÁÊ:K¿ìY …F%¿ÓÐ.`æt¿¿êŠ?åHD¿å³JEžpUNASNone?ï¿tüÒ@Õ?$^pØ$–?€"ÀËoÊò?$^pØ$–?ïú(™V­?l¸¶¿*pw?G—]š¥Mü?l¸¶¿*pv?î'UÕW=?1°ÔO?§Ú¢ª"?1°ÔM?ïØÓãY§Ž?aLƒ€‹«?s–S,8È?aLƒ€‹©4FGL J1602.2+2305?åE8ãwI~@GoîN&ԀÀ:ß­z!.À<¯-‹S…¹@7ö'lO?ú½S,;d?ÌE}x%Ö~?åN•ÄøÂõ@˜u—5@ Žˆny?îE6̤¿é'ص8['?·SëåkÕ¿áçÁŲ§¿íB8¿d.~¿ïᐼ{UNASNone3FGL J1601.9+2306?»‹¥xâ&A?˃ˆ¡;Gö?쎋Pã»7?˃ˆ¡;Gö?² Â¼%r?Áð‹¾Çê‰?í«ç¨{QÁ?Áð‹¾ÇêŠ?ÅÒ»\#tD?°y‹+¢ò?ê‹Q(÷"ð?°y‹+¢ò?¬»\%¿£'?˜ÿ*<;•)?î4J=¤Ç?˜ÿ*<;•)4FGL J1603.0-4808?î&q25ɐ@
ႁOùÀ9bžÕB½À:êæ0K!g@ìfOë$Ò@¿ãzŽ;˜?ÒLóc9‹<?Ôâ¿ù&È@Ù
By!T?ö>~À¨?ïûüР–ä¿âÝ|²ÙÀ¿éåïaLK¿è8«bnà¿íxrmæ¿~­C¼å›UNASNone?áڮljc?Ð[²]{é?ÝøJ¢pí9?Ð[²]{éœ?Ö|2N@û?Õ*›`¢o?äÁæØý_ƒ?Õ*›`¢n?Ùõ#‰ƒM?ºØ¸4™õ?ãn;>Yr?ºØ¸4™õ?¨}W›nP?"»¦Ì
úf?îx*†I?"»¦Ì
úf4FGL J1603.3-6010¿ÚNA‹p…À̎ï¬.À9Í,Ñb¨À;ÿV?§µ¼@+~d	û?ýù™cé´d?ÁeFc¡?ÔÓXl¨ŸÇ@Ëï»@öצÅ|!?ïõ(5©/9¿}-©Ë.ÖÇ¿Ùä½ú¢É¿Úu»Ÿíq¿éõH·(ö™¿ë½¢yMUNASNone3FGL J1603.7-6011?0ЫÖÜ?Q¹péw[?ï~yz§I?Q¹péw[?®N€Ëm?³ÒVP^C=?î«þóJ?³ÒVP^C=?À…
§°Ìs?®~ßó;y?ëÞ½VÌã?®~ßó;y?¿=ü(Iõ?Ÿ(´`\ˆk?ì@zölj?Ÿ(´`\ˆk4FGL J1603.6-0451?ìóþBÔº@@ÒÒ¡øã¬À:<‰œÌTÀ<
Ê©Üݼ@3»QzF@ÆH@áqŸ?Å|ˆÑm?¸­z÷íâÇ?ò9,qx@fº¾'â?ҋ¢cAÄ¿ä'|^ö/¿ä‰}+¤É¿æ•ò—Ÿï¿èÒŠÝ>4¿ïýýâŽlUNASNone?ï6…a˘?'½¾èAÙ?™/^óƍ
?'½¾èAÙ?ïÈ	ú8æÓ?5矈Y¶?{û㌖}?5矈Y¶?î­£ÀCPŸ?˜?8Š%?¥%ÃûÊö?˜?8Š%?îr–ÕŒ£?Žfz6,?¨Ö'§5ÏÍ?Žfz6+4FGL J1604.4-4927?à#‰AEÑ@Àù²%À9:×ÑÍnÀ:¡²okÉ@18qÜf@26~AN?É
¢Gèø?Ӑ±þë-
@gȖÝ@=¨ø1TŒ?ïáâ"o?îƦ!è2.¿ãZ-þ•ò›¿èòbüO¿íRC™²Ä
¿ïýÚá¸lCUNASNone?Ó°:µ\Ã?Éj\žy4?æ'¿b¥QŸ?Éj\žy4?¹?Êæ(¹G?Æ@‹Þ…?ìØ£:è×?Æ@‹Þ…?Ôâf{Jӂ?·ª1»Ç?åŽÌÂZ–??·ª1»Æ?ğ⸐%f?±ÓDÃ'ã?êØQÛö§?±ÓDÃ'ä4FGL J1606.2-4602?¹%ˆPRmo@7 ÜïYÀÀ9üÒhAÀ;'²køvŸ@‡,ÓH@éi]'¬?×s]á~?ïÿ®2D¡@öà鳍@˗P=Ê?ïäžvx¿Ú'¿ó v¿é¥ø']<ò¿ïÿB€X*¿èt—1š­¿éØAŠäËUNASNone	?×éÄbڜ?Ñ´V5z´?äΒ±þ?Ñ´V5z´?±ûML·»?Àu¹<`AH?íÀ–VnI	?Àu¹<`AG?ÚIDiêï?»"ü.¦ÊÁ?âÛuÝË
‰?»"ü.¦ÊÁ?…èÆ Ü?yýNL\Á?䀹\ç|?yýNL\Â4FGL J1608.4+0055?ï²É4ì@Bà~ZxòÀ:"€žP¸À<<g/ºï@lpÕ«Æ@)´Â&?Á">ï)?€» ¹Lé?ÁDŸ—4@Ì}EPC¿¦~ƒœ4Ý
¿áÄÁ/à˜\¿å?ÐÐgŒ¿é-=%$}¿ïˆ3
‡¶?ë2'¸#È\UNASNone?ï²ãUäÉA?Ûyªµ{?ƒG*†Í¯å?Ûyªµ{?ïã þ±?y?…™pÁH‡¾?l_NÀ…ú?…™pÁH‡¿?ïJWÖ÷x?ô5L?–µ!üç?ô5L?ï©Äoý–¶?wc}Á%4?…ŽäšRH?wc}Á%44FGL J1608.8-4803?ìõU™û?i@"ÛÄ·UÀ9"¾®&˜À:¸Gõb@ÎfæÀ@—G½-óX@ëMý¹Ô£?ߛ9ÂC†è@ù¾$"]??úܔîZ¿àû	á€8¿ãr;ò•í¿çiŒöóçÄ¿ï8ÜÀ_×?ÕH߂\L¿ïù"–,ýUNASNone2FGL J1610.1-4808?鞟Ÿnö?ÎÃÞ{UJ°?ɅƒÁ'D)?ÎÃÞ{UJ°?ÕÛg½?ب;ò§´Ä?åp'~Ì!€?ب;ò§´Ä?×Qú³|?¼¡$Êdz¡?äצAò?¼¡$Êdz¡?×¹37Ý(¨?ځ»Ym?ä#fdk¬?ځ»Ym4FGL J1609.3-4326¿ì¤rKÚ@c%}h
«À9ËǐíùÀ;[¦?šIÃ@	àÀõ~@ɎSë9Ÿ?øS"¢Ù´?ÚMú^ÖO@ŊžT~@zYWµ¯?ïÕ½Àƒ¿éÄ#°ß0}¿èb­ß¡»§¿çÜ$X¤ÜÄ¿ìFö£–¿—ß~øzòÝUNASNone	?ìÍ.°ÙžL?½þ׿p
³?¹–Šy3
¤?½þ׿p
³?è*Ó¤¬¹?ÒOý/;^ä?ÏT±mM¼?ÒOý/;^ä?ç¨Ñ–‡‰?±â»«Íh?Ю\ÒðíÉ?±â»«Íi?é/Ôv–Ë?Ámd'¾û?Ë@¯æ%¤×?Ámd'¾û4FGL J1609.6-4837?ï­úµº@rï
åÀ9Ú'(böÀ:•V|
—˜@wh&"ùú@FxõŽ?Í2×XA	¶?д䣮…@ÆeÊÞ@[¤ÍOA¿ëLA³Ù?ïŸá§Oe¿çì×Ï_ND¿ë%5C®«¿äj)i…Õ—¿ïÿÿÊPËUNASNone?åu'öl5?ÍÇ&èën?Õ°'Ӗ?ÍÇ&èën?Á5HV]¡q?ÇÄæÕ~?ë²­êh—¤?ÇÄæÕ~?Õøž(m'°?·µ=ÑFšn?å°ëÉ>¨?·µ=ÑFšn?ËrHŸŒ'œ?·Á*ô0ª–?é#mØö?·Á*ô0ª–4FGL J1610.3-5154c¿Úž—Ø«œ¿Í@,ÀÓÀ8wSŸºEÀ:óøŠÀ¹@tœ…\JÚ@z–¹ëH¹?Å54?LÇ?×6a7R}@jaâs'?ᝄƒ:'¿îìñe2‰À?ïòË.g˜¿áõ³Á
&¿è§ØVmÊß¿íûW>«6z¿ïüD¿L±‰UNASNone%?Å~€0øVó?ÔYöê*?ê _óÁêD?ÔYöê*?ˆ!úìÌ"?¡e»¸ð«?ïŸëxLÏ?¡e»¸ð«?š*wÀ.7?''«d\€ó?ï.¬Gyþ?''«d\€õ?›²Ìƈ´?'	5E8?ïÿ#"i™Ë?'	5E84FGL J1611.6-6013?Ó½8JCkÀ»<ĬlÛÀ:ïÁÄ[À;É°pçÊ@Ö)ax@@•sd{ª›?Ðã`¸vÔ?Ö£²A†24@hXJb?õq	̆+?ïû?¤Á¿ëž'ŒŒÁ¿ÚÝFA­ÊS¿æ¾Q€ž¡¿ëV8!ï¿ïøžý†¨üUNASNone?觵¾HF
?Ƨ§0,6e?Ía)ÞçÙ?Ƨ§0,6e?æƖ'X¢"?ÒìžÂÔV ?ÒrÒÛNºØ?ÒìžÂÔV ?âí##ªZ?¸‡Mƒ{Ø?Ûà%¹¸«J?¸‡Mƒ{Ø?Ñ«T®fã^?®Q^»§?ç*U¨ÌŽQ?®Q^»§4FGL J1611.9-5125c?µÜÕBlÑ£¿¢ÀòyÌéÀ8$¹ØÔBÀ9Œûµîcö@xOE¤~@ŠQã!¢è?Âô`$-ó?×ÅäêÑ@"8]>Ÿx@\ÏRc$=¿Ï2¾°Õ?¬£"Šùï¿ãW榒¦`¿é'š¡×U½¿îûs®çŠ¿ïÿcøÍܗUNASNone4?{º–ï?°VŽÁlä?ïȊÒ!ß÷?°VŽÁlä?j#iJ?¨ùÉú5Ï?ï|®ä·N?¨ùÉú5Ï?vPçfb?‡ñ÷nù$?ïŠ&¿Äbf?‡ñ÷nù$?`À"ÌüFÏ?Sbß÷qlu?ïï?k3¹?Sbß÷qlu4FGL J1612.1+1407¿í:å2éº@DÍÇ%ÃÞèÀ:†w-^À<ÂÛpÔ~r@Ü0Âë?ú†ØF}'Ó?ÇëX¦4]?æö·¢CC@¾1)?÷ä‡ÑÆÞ¿ïÿþøþ"?ïÿk»9ýR?»"òm›9¿âòq׳°œ¿ìÐ5½Q.Ç¿ïøœ>9¡ŒUNASNone3FGL J1611.9+1404?˜KàÚßu?«ý_Û""?ï= ÿé)?«ý_Û""?—³Á{K?§$ßÁíõ?ïGÔaô%?§$ßÁíõ?¾è¹×éW?¨À&lGìK?ì?èÅÕ?¨À&lGìJ?p '@÷}?]66i.÷ˆ?ïÞ¾ûÝ~?]66i.÷ˆ4FGL J1612.1-4526¿ìªG¢m/@5àqÅ?:À:"Ëùh6JÀ;ffÓs¯û@geÀy,g@Ý`#Up?Ùª\²½­?âH«4̐g@dϝ,@ 4¸ïJP?îÂOpV¿ä?3ÞLQ¿á'ˆô'¿é¹È®Zÿ¿ïý¸AûM¿ä²@Äì-»UNASNone	?àDä2›f!?Ð2Föëöu?ßv7šÉ3¾?Ð2Föëöv?ÞqšgÑ?Òہ'mEú?àðÇ~²Ì?Òہ'mEú?áŒ7H毷?¸
je1ƒ?Üç'n2 '?¸
je1ƒ?àÃÇ,‹?¶‹æ³\¡?Þxq§àéâ?¶‹æ³\¡4FGL J1612.4+0409¿æ·ÿÈùP‡@Bu"úÖËSÀ;Ÿ$`2À<±ÑtÒ9ô@ò§´i??ü¼˜6Ã
¬?϶ÊÂ["¶?Ø×@	,LÄÔ°Ç@+e¢F;?ïæ'j(¿âûjÚim'¿Ü&ŠwÔx¿ÑgïØÓÁ¿í
â18¿ïÿ›÷Aë]UNASNone?ïøûÀA­?TÆúû¸8à?OàþùL.?TÆúû¸8é?ïðÁM¶Ñç?tžÇ	?^}d'\1e?tžÇ	?ì­qð›5?§{'v}W¢?º"s{&W?§{'v}W¢?î»LXOh?‹m~K`ûü?¤K>{	s?‹m~K`ûü4FGL J1612.4-4419¿îzŒåR±@MhÍJ¡À9êIHHn.À;7oE298@×ÆÎ0$5@üa'?ÕГÁ=w…?î÷‡ Q»@ً÷ðg?ü›è~Y!¿ïø罓ô¿?ïï"Áhj£¿ë/¿5_ˆ¿æúÖ?½/K¿Üõ™Ÿ£ÉÉ¿ëþ!²WVUNASNone?Þ3{'´…?ÔtÝÉXÙÁ?àæqB6¥½?ÔtÝÉXÙÁ?¶õÊY¢Ë?ÄDµúÇ*?í!F´Ë¼f?ÄDµúÇ*?Ù­pšØZÝ?º…h'ê¡?ã)G²"Ò'?º…h'ê¢?Qܵó>Ó?b~Œ	
C?ï÷¥`˜?b~Œ	
C4FGL J1613.0-5102?Ý0þ#Œ¥ ?½ò6=Ô¢À7Ù¯ÅU	GÀ9Š¦V@~u@ªŠÀbÜ@r.þñG?¾Ì¡Ù¯l?Õb'|ñ˜3@¯ªŠ'¥a@ ¨²fD¿Ò[—?ø¡¿âG¦Ý¤áK¿à—à?ñ2¿è›U%ÌBc¿ìQ'[¶¿ïþ£^"_ôUNASNone?Š~
¾y¼?°oQ{ۆ?ï–ûÉ?°oQ{ۆ?Š™»Áx—¶? %xK±G?ú¡? %xK±G?¨™J'¹t? ­\m,?îvkVïÄh? ­\m,?m8üÖ[oX?b°¿JTp^?ïâÇ)¤'?b°¿JTp^4FGL J1613.1-3840?×íAG¯Æç@"$§Ös>¼À:°ðs›OÀ<
N‰Ðκ@ ø*$Á«\?óDJè[žŒ?áŽ-àc­?àÚ;ëh™G?þ1ßÈR@Ž¢ÛÔÊ?çZ,Ñð"<?ïxe!Aï¿ës…hŠ-?²(þ¦ä†¿Þ……zþ£ß¿å̂$2pUNASNone?îÀþ/¯?²;ÐtÊÛ?£ð-?²;ÐtÊÛ?ïßØ%,"Û?ŽS¼½\X?píiµ'ž?ŽS¼½\Y?í*µ‰I7+?¥-ãº?¶ªSµ¶F¬?¥-ãº?ï"QòÏè'?}µÀÝES?ŠëƒLߎ?}µÀÝES
4FGL J1615.3-1512?ëK¨]"u@8è"Ýz™úÀ:ŠŽ]%uÀ</j£	@­w'ÃiL?þ:‹KøüÖ?Òf';‡?Öó{!ßMÙ@f"f\Uk?ÿáJø÷£?æ'$óÅ¿æ´2ÝeK?çè?º*2Ù¿å6<!ÄJó¿âõ@S­&>¿ïþ¿UØUNASNone?îËóD~oÅ?£(¨(y?£@˸¼?£(¨(y?îåXåR?µí˜|¹ ?¡§êqªï?µí˜|¹ ?ë]zæDê?­Øxp+nS?ƊfìV?­Øxp+nT?ê&¡©ûϜ?³&ooÏv?ÇeyXÁ?³&ooÏv4FGL J1615.5-5434¿ïÄÝ)ý32À¦°'ª¸À9á÷¯îpÀ;Fʨ/^'@Êx‰©@'ì®êc·?Çîüâê?ºd Ïª?ðxºvˆóY?õaDì³r?G)Š=¿éG1b"´á¿ã
'ž*x¿èVlˆ¿VÿáÁ*l»>¿ç+YnLUNASNone?Ãä™?†ô×Aªp?‡XÙî?†ô×Aªo?핋áe¤ð?ÁMÏÃû8?³S ôÒ؇?ÁMÏÃû8?íqDèZV?£:»ã}5g?´uØ¿Ý-R?£:»ã}5g?äåÁ;?¸Üƒ2+V?×Ø4}çù‰?¸Üƒ2+V4FGL J1615.9-4322¿Â]VH()@N0DkjÀ:"A±{7¯À;jÃwï%@ÀØ#B$h@8Omü]?ûéM¼KuI?εN+>?úzDºD4@ÜCR:4"?ïb<jêY¦¿ß	?"OZ†¿ë'ñ¡îQØ¿æn~ãµÇ¿Ø°†zØä2¿êƒËf›?ŒUNASNone?æ',œJ{ù?ÍmL¶qkJ?ÒݦÇk?ÍmL¶qkJ?붅`«Ç?˔kh,ç?Á%ê}Sˆç?˔kh,æ?棻Y=%?·®†Æ൫?Ò¸‰M…ý¶?·®†Æ൪?îaáµYô ?¨\2©2ÂH?©áäª`¾?¨\2©2ÂH4FGL J1616.6-5341¿ê@É)\ýfÀ[!f'À9]ħd]À;Ùô¦/ª@@§.­'@›Ç »aj?À7™NÆ?ïLùx&'K@!Í¥¹bŒ½@Ô+Ž#CÒ?ïäiÁºŸú¿Ýƒÿ°É¿½¼dãoü¿èŽ?{¿î(ÀþãJh¿ïÿUJÃUNASNone3FGL J1616.8-5343?IÃQ|è?RQï‡Ð?ïù+¿`Ç?RQï‡Ñ?{JY‡oÍ?'Ùá¥æ…?ïÉkLñ÷!?'Ùá¥æ"?"…š4iÚü?ˆ¾MGœîE?ï[Ó.\±(?ˆ¾MGœîC?iEÆÕô>ü¤Uù=?ïÿ'Zèç">ü¤Uù=4FGL J1616.6-5009?ïêÃQ¥·Œ?×ٜSˆ=QÀ8LÀ½ÊÑJÀ9ÍLê"]ð@ À‹–!@ë|þX`?ÉtAEo Í?á3Ï@ŠÎ-±ê?ò!#"'Ä?ËXòŠv'¿Ùµl]÷,¿äM: ºË¿ìZŸ2ਿíTi¿n¿ç˜Þˆ¶óUNASNone?Ì2JF!D?Ö:Ø
£Ýž?èómnx÷®?Ö:Ø
£Ýž?"Vp·2?¬'"\êÙW?ï]LOòG?¬'"\êÙW?²ÙîIØv?©Es´æ?í­äÂ6Äò?©Es´æ?BÜ>p%??'pˆ"KL?ïÿé?'pˆ"KL4FGL J1617.8-4418¿àûÌÉáÔH@­ò>v]TÀ9é:G#«À;všÛ¸ù@9(_D´@=˜¿p?×è^"Ë?ïþ©SK¯@ÿSŸºE@£ñ~Ý֊?ÜÄF€íÑ)¿ÔùQ$µÁî¿êQˆÞ¶YC¿ïþð g?ï(J®kc¿ïý¬2ùQUNASNone?Ããø®ËC¸?Ƒ}™mC?ëÔM/?Ƒ}™mC?Õç'7fs?Ù$öÿ{J?å7d~LÇ?Ù$öÿ{J?×öÆÄé¶?Àrý•^î?䜝‹|¦?Àrý•^î?Þ}°n°?Җ›ØÊyj?àÁ'üõȨ?Җ›ØÊyj4FGL J1618.0-5119?çÞÚ`u¿¿ä3™Š€!#À8aOZ±&~À:`ÇÀôQ@ ®¤¸Üó@¢ñÄÓÚ?Ä©ò­1&?¹UJ4VžÈ?ü­ÚB×@›cÇЎ£?êÐxR÷ô™?èD
úú?Èrè•U<H¿åe»¡k5¿éDù>oÒK¿ØøÒy´÷ÄUNASNone?·ù—Y®¥?Ã\NŸÂ?í ÍÊ+?Ã\NŸÂ?ÐVŽrK%	?ÔIYNàö"?çÔ¸ÆÚm{?ÔIYNàö"?ÒhæsÝ?ÆÐ
œƒ?æüyˌÆ?ÆÐ
œƒ?Պdþ3†¼?ÃW›n+ï?å:̀æ<¢?ÃW›n+ï4FGL J1618.3-4537¿ï«¨c_@RÍÀÓgÀ9Úl <K
À:#ÍbôÁÞ@渭Ûð×@ݺZÚA@m">5ŵ?âm-êñÑ@»†Eÿ¾'@¾n¢Ÿþ?à‹)ßwtV?Ú÷;ÀöTÛ¿ê±­ÿ"Z¿ìaÄ@6Põ¿Ñ/AÁÁUö¿à3½Ò^FUNASNone?ÏÐì@á?ϸҪtHk?èøïýÈ?ϸҪtHk?ãÖBφ{?Ø´läG?ØSÕz`ó	?Ø´läG?ãBrrež0?´$ZV?Ù{4à?´$ZV?ì ããU»?¿ÉíÇ6s¶?ºøàã•R#?¿ÉíÇ6s¶4FGL J1619.3-5047?ï[±VF¾ó¿Ø¸"*}ØÀ8¡.¢ªºÀ:¸ÒD@ƒ8XŒ@x@@aïß?Ë"">Ä6?Û²Çë¼|@®ˆã—?öþJ«ŸÖu?ÖîøüU¦{¿ålÿ!³®ï¿ÜkñUBQ´¿ç…`'¿í«a­šž¿ïrBþx%UNASNone2FGL J1619.7-5040c?AŠÙ‡åê?±Ed*cƒp?ï}ó©3ÀÑ?±Ed*cƒp?žò
Jk›?±¬/f§?ïxo•¬¤?±¬/f§?¥•4Õ´7¡?™aöXâhÈ?²¤¼…?™aöXâhÉ?S Gð¤³ß?CÎñî77í?ïöoÜ­¦?CÎñî77í4FGL J1619.4-5106c?í:ôûyÈ¿ã°™?׆dÀ8=³/lÕÀ9×Ô)¸`.@!GÁntÒ»@'PǙ?Ñ
\^ûŽ?À½y]9!@^aµ&¾?ý|V[?ïÿúŒ"¸'¿ãP'7§¿ê"qh"¿ådÀÉß2¿åҗ¢¡§¿ç®ÿ\lUNASNone$?âü©K¬?ÑÀÁ"µ·?Ú­iü§ã?ÑÀÁ"µ·?½²â'µ:?Èä$rñª|?ì\	£­©X?Èä$rñª|?ÔÀï4${?À¡ïTѝ?埈eíúB?À¡ïTѝ?§Kó«)Žä? N=¼D<?î‹@ÅMg? N=¼D=4FGL J1619.5-5014c?ïn±SšK¿"ˆ&ÌêÌÀ8ȽÇvK·À9»òt&BŠ@ÚhŸ{°Ð@cnda©h?ʺðViÄ?И¹à6*@
Þ ²'/@%'~È2¿ïH¤´Îí?î<|½ÀÀO¿ØbO §)û¿ä†ÞvB||¿ê™XÌIð¿çï7@-ÌUNASNone3FGL J1619.0-5014c4?Lj…ß9Ÿ?ÎOÓÐÀÈ?êވ:q˜?ÎOÓÐÀÈ?´*Ý?
	ª?üú²à÷?íz¤X^Ë?üú²à÷?Æ?ä&üË?²ú–B'ºå?êz0ö@Í?²ú–B'ºå?ÏéEš}"Å?¿C¥hÒ16?è®™`šÏ?¿C¥hÒ164FGL J1620.5-5729?¹\žÈ0vÀAÄÆnÀ9ßÊKM
À;‰%Þ¶Ú@
œß^@†{¯£Ç?ÈP‰°B}?Ægv[Ñâá?ÿòŸ	E# ?ÿUûƒ¯?ïˆ&_e@L¿Ô
£\ú¿æ†Ž¾`¿è"Ø¿Ÿ<Ç¿éâ<›<¿ïþØ
bUNASNone?ç'È$ª?ÄU֖u&?ÐûñÄo¶¬?ÄU֖u&?ë^;üc?Åé	Ú̧ì?‡çs?Åé	Ú̧ë?æn¡m
¦?¸	–7ˆ?Ó"½û%ä²?¸	–7ˆ?ãê6³wý#?¯[ÝW'c?Ø+'™º?¯[ÝW'd4FGL J1620.8-4958c?ëzî­þo>?k'Úæ@À8s¼W3Ã|À9¤2ðîE@ÁÔKòç@Gòš¼¯H?Å2"{€ê?Ѫ¿±±=@€Âa8ÿü?ÿÕ©$|>¿î/§íå?ïoÑÿ¼Ž;¿â=à‹F¿ç˜§Å¬G¿ê–±‡Ìè¿èÈÔð‡½UNASNone0?"¥cåÆj?¹KY°ââ?ïZÔçØÑÍ?¹KY°âá?'L~U¬?¤spCŸ?ïuœ»R?¤spCŸ?¥-ýo,[?–¸í'½ÜÂ?î­ )
>Ë?–¸í'½ÜÀ?"Ëy8‡Wv?ÑD>ÖH?ïa¤6;ÅE?ÑD>ÖI4FGL J1620.8-5035c?ïÒæ¾múu¿Ú¦lü,¶ÂÀ8A˜iòÀ9Ð1T5â:@!
"é3_Ô@¥ŒÄŸâ?É+å¶þ"?¾bcL€Œ,@Œ$›À»G@¨³Åê°c?嘱…K.?ÏÌ
…&¿æë%(®u¿æÆÕ½â¿æ5þßÄv<¿æU‡Ô>UNASNone4?ÇÑî¸ëã\?Ðx;ì~?ê"QÅ)?Ðx;ì~?­TðT[±o?¾1¼hæ´?î*°úºDé?¾1¼hæ´?Ê30ä3ôê?Ã÷oW¿?és3ÆóÅ?Ã÷oW¾?¹
oc"·†?°–Ò÷Æ?ìÞR›©?°–Ò÷Æ4FGL J1620.9+4852?éòŽËUñ@F>dÜY2À;'òvªHÀ<÷#ý5Je@4½ú¢É?ÿ‡ÝDUG?Ñ+ä<U?Ç#õ}›?ôý›yÙ
@·]`XZ_?ïÿþÞ÷¿í­x©_	{¿É£èg‡ù‰¿Þï0ês¿î
▸"?ØËWí»°UNASNone?ïûȎTäZ?BÄ%xׇë?@ÝƬn•-?BÄ%xׇô?ïúJˆSCo?k1+Ú
+Q?FÕÞ²òGæ?k1+Ú
+S?ïØ2#|?"It/™«ü?Ÿ¼dù»}?"It/™«ú?ïÀDðt¹®?lÉi+‹iÇ?݇ţ(ž?lÉi+‹iÇ4FGL J1621.0-2625?ÖÞ]1ß@0sï¿@PÀ9ÆÕ©²ìÀ;t	§H®Å@»¿Nßáý@÷d[ËÙ?̈́Q2øzÑ?Ø"@Îé@‹6¿y@*ö'©¿ïê~ŸBP?ïÁ0αÿ¿éåϽ—ûŠ¿ç¸ˆû¼¤¿ï»Þ§j¾¿ïÿö$´ë/UNASNone?禕¯™›?̄ï€gH?ÑβԠÌË?̄ï€gI?çA6¢Ü°?Њ´³7½'?Ñ}'ºGæ¡?Њ´³7½'?àw¢ãÄù?»›™y)º?ߺ8Þv?»›™y)»?åqÞ <?¸óäýb?ÕB¿‡óê?¸óäýb4FGL J1621.4-4511¿å4kž­."@
ª}>ïÿØÀ9ºÜ€žöÑÀ;n4Ïë@ï²>+3à@lX–š?Ô§]7¼?ÔïŠ|p>@O@4£v@+
y*¹<¿çtí²öaò?ïҀÖT5¿æÔÒ$ú¿â
Ÿû³j%¿ïÿyÈBúQ?î"ò¨ÿh+UNASNone?ÕÐ40¨´ˆ?Ìî^rhÁ?ååç«¥¼?Ìî^rhÁ?Öµ}ÐÇé?Ôˆæùؘ?ä¥Ar—œ
?Ôˆæùؘ?Ö;=•ì?¹Z<;UJ??äâ~a5|
?¹Z<;UJ??âG¸"G¾?¿Îzvé?Ûqȏ»pƒ?¿Îzvé4FGL J1621.9+6706?ßP×Mª¾@C‡á2µ^òÀ;.÷<À<§]k"@;rW3C@§ÒŸt¤î?¿ìðXõ¿ºEik©q?ðÌgL?s³?÷,¨‡ª?ï͎É[ÿ¿êÙ"±ð*¿èÌÝÓ/g¿à‹ èBt¿ïüQ¿æ4}¿î¬é!í¸UNASNone?ïãå3´ü?qé頚-M?lÌéKC?qé頚-L?ìèNúá?Ã
×3Q
Ü?¸¿Íˆ/Pð?Ã
×3Q
Ü?ïW­Bá؊?:	ô¯i?•
W£ÄîÂ?:	ô¯j?ë.»yÔÂ-?±¸BlÇz)?ÃE¬÷M?±¸BlÇz*4FGL J1622.0-5157c?çáëñ©š¿øÓíçÐÀ9mbÙéìÀ:´&Nyá@䉱ïý@ã¬BÊ?ąÿb$?Á	WC¡ë?ýö5{âÏn?ùDÔ:ªJí¿åvw@(d"?ïâÜ~E«0¿å`i,"A¿åFÁ+Xô¿ìÞJZƒÚ¿½Ãø<èÎUNASNone ?Ø`AÖÒüð?Ï|?þ—?ãÏß–ˆ?Ï|?þ—?à:MêÏÙ\?Õf</Z÷?ߋd*`MI?Õf</Z÷?á7Ó³mÏ?½Ø˜£É?ݑþX™$b?½Ø˜£É?ËcOª?¸=iÅOF?é;½',_?¸=iÅOE4FGL J1622.2-7202¿íÀ':`ÒAÀ/þKZÀ:}"ç¨ñ%À<|ɳ<ØÎ@¹âÖysß@$  0÷ð?ÂZŸÞ­?ÕðÖâz^@[è¡>©‰?ùzÛž?ïÿÝƒ(i¿ÝæüÅW8¿Ø¾\ý1§¿ä‡(mÀοì¾}ÖÅt¿ïÿ¤?åÉUNASNone?ÄԎ߫ŽÓ?¿ÖíëÉU½?êÊÜHK?¿ÖíëÉU¾?ÉüAÈîžh?ÎÅíf«ò?é€ïÄXf?ÎÅíf«ò?·nPR]üh?¥âw5w€£?í5õ´@s?¥âw5w€£?Äá´ÍT9?¦[?ØÒ³?êüǒ̪ò?¦[?ØÒ³4FGL J1622.5-4726¿ê'mí±÷Œ?ùý ½é¨À9V3é;˜À:²xþŸ3@®hÌr3ú@tÝdʄô?Èë¨Z&½?Ïl¡ÿCÂx@Ê:#}?ÿx-
TQf?î˜ÓÁ2º½¿à´Ҟå¿ç€ÔÜeÇ¿è¡Ý4ùÝ¿éTô¹zàq¿ï¾á77¥UNASNone	?¹Ï¢5v2ð?·5ÃË«¹?ìƹQ9¢?·5ÃË«¹?É»æ¨`?ÎðÏ%«÷ú?é'Uú§ù?ÎðÏ%«÷ú?ÑMU둴"?¶®Ø&Ù%½?çYU
7%¾?¶®Ø&Ù%¼?śkÿîì?©äþ°Œ"¶?ê™9%F?©äþ°Œ"¶4FGL J1622.7-4934c?àZkÖ$q?·†×J)CñÀ7Ò'D:ÂÀ9bÙéëÂ@J2Œðø@‹$ÜX[?Á5šìð?Ô¥lÞ@9É oâ?üç`¬"{¿áø"0¤º?î[R¡ƒâ¿àZþ¾·`T¿è+Öþ)E¿îW}à€ˆÑ¿ïýÜÚa
UNASNone0?Š‹IV?°¦ŸBˆ»?ïÁßÜêén?°¦ŸBˆ»?}¥;:°u?"ƒÀ¿ÝÚ?ïĵ‰ßŠŸ?"ƒÀ¿ÝÚ?Šº^˜Êoi?€d¤¥d³?ï•…œÖC?€d¤¥d³?7	¹'U´¨?.…¾¤q=?ïýÈÛJ?.…¾¤q=4FGL J1623.0-4624¿ïŠ˜²‹¢@Fb\ìj!À9e3ÔBâÔÀ:àŒ]"Y@†zº±AV@ÛµûÏï—?Æë΅3±?®[!3‰ù?íºüÀ°^Ø?ù>&×/QQ?ïº8À»Çl¿ç*.<Sme¿êú©u°¿å>`"†É¿ç–&ÇUj¿à0«¼²UNASNone?í͘Gßò?´ž²±oÓÁ?·A"=Áp?´ž²±oÓÁ?æ-jKþ,?Ôïô<™Ö?Ó¥+h§Å?Ôïô<™Ö?ëÙMÕLÐ*?«Ê)3k	?ÀšÈªÌ¿Y?«Ê)3k	?⅌Wê"È?¹‹GL®1?ÚôçP*Öo?¹‹GL®14FGL J1623.7-2315c¿»³ì>U*@2"ëÄØíÀ9»øç
¶À;&ߢ'fŸ@_ºžLè@øb9°û¶?¯1†_Õþ¿XßÜÛO?´ýò^¬³¨?ÿG[iUŠ¿æˆ®Êä?ïüœh€òÚ¿ç%Ž?w4¿élëá:(¿è¢™ó[¬Ï¿Ú‰=UöØUNASNone8?í¨ï"äîo?²Îî¨.7Ú?²¸ƒX،'?²Îî¨.7Ú?îo£ñ'?¼QÚbMà?©EÏÐçæ?¼QÚbMà?êœû綉?¯YmŽ&ú?Ōc™%Ý?¯YmŽ&ú?íëÀY–†A?Ÿzo%¥?°¡ý3KÍý?Ÿzo%¥4FGL J1623.9-6936?åä/ŽÀ+í²'¸#ÈÀ:]½‹ç)À<uƒ/ÊÈç@i"¨ò?ÿãf³"@?Âçښ?ܺ?×€
Qh@~3Auì@F-ðS:?íþ'›ýø?ä:ÿ°Nè¿Ý¡ªÌô»¿ßBL`€É>¿î9ÎWçG¢¿ïÿÚ«² ÒUNASNone?ÕãbP?®?Ǭ#t¸{æ?åN×ú`)?Ǭ#t¸{æ?ÜDç"/?Öb"yð¾?áñ݌=÷g?Öb"yð¿?ÅwŠcƒÝ×?²òƒ7é=?ê¢gŠ?²òƒ7é=?á4Ví[Gç?¸>øøŒ?ݗR%Ip0?¸>øøŒ4FGL J1624.1-4941c?Ü1	0/û¿Ã½?æõÂåÀ9eôݍqÀ:ß`ݐi@¯ÈV"Õ@Û`
†Ñ?Ò:Ùâ)U?ä_Ä@Œ70@[®¤Ã™G@!­Ý|é?åÁ¡ŸØx¿ê"ɞoc¿Çnיå¿ã؀_5ð}¿ëæÕÂ>ÔQ¿à¯ÖòÀ|\UNASNone2FGL J1624.0-4941c0?¤œÎúê?²¡:õH?î¿®V3R?²¡:õH?ÏNqœ…–?ÒI²l¢Ò±?è,c˜Þš}?ÒI²l¢Ò±?Ì௣—î?¶z (4T.?èÇÔ>"?¶z (4T.?Á"F<õ®?§rØ[)÷?ë¿Zîp"?§rØ[)÷4FGL J1624.1-4417?ÐCF@
—Ne¾¡À:8;fÀ;EÝhüBÜ@äÀ^g@ä…BÊë?˲&˜Æ
?Ø/s?è£B@WÝ¢&e?÷s7µxó1?ïþsè¿ãã'ö»3¿ÛØ´¢¨ñ¿å‡ÐO¹¿íهÆ2~Ø¿ïùñ]¥Í…UNASNone?Ð&ó—*ü¨?Å金?çì†4j¬?Å金?¿>m" º?È9Ä»~úó?ìØ2Okè?È9Ä»~úó?Î`Òm5&‰?³ºë0+€?ègËd²¶^?³ºë0+?¡™Ü,á?†£ÒU.Ë]?îæh8
1?†£ÒU.Ë]4FGL J1624.9-4538¿â­8Á»Ã@®ò"z–À9½ï}Ѽ÷À;)²ì`@ub
fE@ܝ 6×?Ó¶@ï3?éDGÝå#@LRç-¡#@‹ä<€?ïñ©ûçl‹¿åø‰|ëä¿àø›ó-u¿îh—c^t*¿Þ}z¿ŽËµ¿ïÿí )k3UNASNone?ÛEÒè<=Ä?Ðøñ±3?â]‹áá?Ðøñ±3?ď_Éz˜?ÏlY9ù?êÜ(9¡Z?ÏlY9ù?Ðîå^Vîå?»:oß0`»?爍PԈ?»:oß0`»?¬~&8s?¥6¡ddÚN?î8ϝœy?¥6¡ddÚN4FGL J1625.3-2338c¿®Ñ;	˜¿@1š'>[…bÀ9éÊ¥«ÔÀ;Î\ïÅ@
Ù æ@ê¬azŠ?×n†ÆX>…?ãb_p¨à@<÷S½@W?	*K-?ïÿwåëo¿å»Û¾,K
¿ç™ö!ãÕ¿ëõækÚC®¿ïÿÿÊPË?ïü!~|UNASNone1FGL J1623.5-2345c(?èâ,L2ãž?Ê»4hà?ÌwNÏ4q‰?Ê»4hà?Õe­){Ì?ÒáŒ8±3Å?åM)kBü?ÒáŒ8±3Å?Üج³öm=?¶)-ôË`¹?ᓩ¦É`?¶)-ôË`º?ÍèÙÆI‹N?¹µóÐE{?è…ÉŽm,?¹µóÐE{4FGL J1626.0-4917c¿§Y¾{EÈa¿¶aTâÀ8D*zýÍ À9Úqvdá+@<†¯Üüñ@)Á'°—?Ë;Á·šám?¢*	é¸ÀÑ?æÕÊ@qà@;†rJuD?áXsÉü7ô?¹¸"늿ê恗DU¿ç!Ú{9¿åŠ*@Ejm¿Üëû¼#‡DUNASNone3FGL J1626.2-4911<?΁õì?ÎFPµêlð?èxŸœ"ü?ÎFPµêlð?èO"ˆ"©?ӕÿ$w'?Î٭ݱ[?ӕÿ$w'?ݱ*vÅ?ÀøØ'¡>?á'jòDó?ÀøØ'¡=?èŒËqor?µjã{œw›?ÍÏðÒ:B9?µjã{œw›4FGL J1626.5-4406?äZW½ë@£&Æ=f"À97RÁmóùÀ:þ›H"@Eªs]@yä"rÁ?ÄÚ^ZÔ6ù?ű9ÉOj@
f H	"@¦+Š¥?ïÁkoº£?îÆ>¾+Ê3¿ä¸R÷ô˜Ä¿âçfá¶hÝ¿ëw¡Aƒ­õ¿Ý+m×sï¼UNASNone3FGL J1626.3-4406?ç møæÊÓ?Æ¿Ò4*?Ñ¿$2jZ?Æ¿Ò4*?è'l#6¸?Òc<´"?ÏbOs'•?Òc<´"?çzåèNçÁ?¶Ô¶­ƒ?Ñ
4/b0?¶Ô¶­ƒ?ç£CuÙå`?¸L®RÕÅ?йyL5??¸L®RÕÅ4FGL J1626.5+6257?ïÿÇÂwŽÀ@Dß°Õ À;j‡È¶½—À=
eÀN@ uVÞ^¼?ýƒ_0Ð?É W£Õݘ?°Bq>±—?æ¨B©È¼@}¿AI¿ïÿÈl뻥?ïü¸¹"Š¿ÊÅ¡ŠSÖl¿å
"Þ|L­¿ÂW$T9¿ãkŸ‹K"UNASNone?ïÿˆà(½?é""È=d?
ÇþõЮy?é""È=7?ïý®,ô^?P&+Ž¨H¾?2Ž˜_Ý	ò?P&+Ž¨H¸?ïËDŽ_µ?€)ôûF&4?z=Ð%}?€)ôûF&3?ïúÜ_Q3ø?7^hi¼?DŽ'»0?7^hiÏ4FGL J1626.6-4251?ïþqšKŒ@>­\ÄüõÀ9«ã°> ÍÀ;
»y¾1ÿ@ÊÅ&@ù5žG~D?ÍpÔ©e«?ӝÁÓÊm@íÛ¢R¦?ö­3²_
W?ïõ=߉'æ¿äS«Èp¿ææq¹€¿®¿æì´ÿP­—¿îí47³K¿ïÿ¤''UNASNone?ày"É?ÍËËUô?ß÷óÕØo?ÍËËUô?Ñލkõ+h?Òãùà°e?ç¹JjL?Òãùà°e?ÖÑ["Óý?µÿÍsÚHÁ?ä—pÒ6?µÿÍsÚHÁ?¬cµ÷@>H?'Å›tpì?î9Ä ‹ü?'Å›tpì4FGL J1627.7-5749¿ÕbúúÙÀȞºjÊyÀ:%µQàÀ;ï 8"«Ì@|T{,q"@‡ŽºB†?Ų`$'ì.?Ûk_ý–™@èAYB@‰,™»þH?ïJ¶Ýw>ü¿Ò^©Ã(ß¿å"áu¿èì]60¿¿ïýؾ°»¿î·Œ~~
GUNASNone?²‹«†¼{ã?ºÚç
!I{?í®Š(pƒ?ºÚç
!Iz?ÂEStA?Ä '¿£ö?ën¸ë"ï¾?Ä '¿£ö?¼ŒÚNÄ´3?¨>g_D?ìnd¶'iz?¨>g_D?¾;׶*¼?™hw.'o?ì=x…	:©?™hw.'n4FGL J1628.0-4920¿Í褛	<¿Öù¦¸&øÀ9¸<ãÀ;^ݚzj)@b6¬j—?ú{à€Þ·±?ÐÎҀÀÚ¦?ê £ylS@2µÖ\?þÃ]¸Aû¿ïþY#¯?î÷Pß@—Ë?ÒO¥¤ê°¿ä}z´ÒD¿ì"{ýýFg¿ïüÂÉ=ÌUNASNone?Á&ÚZa"H?¼y;Ic?ë¶Iig›-?¼y;Ic?¹í#8w¢?Éæ‹ÎŒÚy?ìÜb[˜ñ?Éæ‹ÎŒÚy?ÌÏQgfQÕ?²wÅ]¡¬æ?èÌ+¦&k‹?²wÅ]¡¬å?¹ŸÓì:€?£Eª£?ìÌ'x°?£Eª£4FGL J1628.6-4553¿ÖG_}áY?ÿ<û¹IbJÀ9DçW'Ž
À:ÔL÷)—©@L;´4ç@]X…Ó8?ÊðΉ»U+?Ë0¼
‡ÃX@2/ãšj@÷jt6?ïëÖï썿ä­úNw\¿åé¬Áêp¢¿åË»Š…) ¿îۚû™hò?¿›šOÌñáUNASNone3FGL J1628.4-4546?Öÿy;Ä?Ê	r~àA?ä€xÃb8?Ê	r~à@?ázݜ¬x'?ÔéãW?Œ?Ý
DƧ±?ÔéãW?Œ?à.DìÚÚ?¹½¨ƒõØ:?ߣv&JK×?¹½¨ƒõØ:?à~¢OZì?¶j'ÔՆ?ß»aJ'×?¶j'ÔՆ4FGL J1629.3-4822c¿ì*Èè‰è?ÃÅR.¸ÐÀ8H00IsçÀ9¸ÒãgC@¼HOúê@zÓOž?ÉK⁔ë	?Û	읢'½@Dh¢€Èè@ÞN«´¤7¿Ì°¿%j?îÏ27Š°É¿æ€‡yÜdð¿ëõUҚl¿îpñÚ£O¿ë8¾"UNASNone8?¢"~\íú?½Ï>¥±_?î׸?ñ!?½Ï>¥±_?ž´§}†??¶!y]w{?ï
ZÇLÎ?¶!y]w|?ºÎÇzÙ?°=UðÁ¦?ì¦'_P¥?°=UðÁ¥?zYî©i™?püÚ1ÊÇ?ïËMÜ"­-?püÚ1ÊÇ4FGL J1630.1-1049?Ì×2@8Ô³_=}9À:™Xù–YÀ<ÈÑÚRÇM@Í_íüG@ÖÝâžÆ)?̳üqU-?ïýò߆õ@ü¥zxl"?þƒÞ©Ä	/¿èQ)/»¯¿ãý›6QË¥?´Gz=ó>¿âWŸ¤¯¿ïÿÌhù¾¿Ú•©Àª€UNASNone3FGL J1630.2-1052?òxú› ?'rKhƒ?ïº6'?'rKhƒŽ?ˆŒÊЂÐ{?" F°ãó	?ïÌÔ½ô¾?" F°ãó
?¹½HL#Ùê?¥ó×ë4ü?ìÈVö{"Ã?¥ó×ë4ü?j+ÎúÖÙX?Vî7ßÔ»?ïåÔ1)'?Vî7ßÔ»4FGL J1630.1-3546?ê.¿KbÒ@!Zt֐›À:o¶Ò"mÀ;Ҋ,l@ .á¿Î@´"¡ºÐK?Ñ¥_ .^?Ø`etÎß@ÿïÕ@Óo¦©?ïýœ
`{¿Þu]¿ä'"Ð=1¿æÐ6y8Ñ¿ïÿÿ)@k*?îÍ<(¥:¸UNASNone	?ìÎT9°?¼Wq@ä¢?¹/í^2€?¼Wq@ä¢?ݶz$Ò[?Ôkþyê?á$ñÂí–Ó?Ôkþyë?Üñ¦+Ç
?¶ô9ß²?á‡,êy??¶ô9ß²?ÜS沊ü>?¾È¬/û‰?áÖ¦ºá?¾È¬/û‰4FGL J1631.7-4826c¿îçn¯xÆ¿ÇYϪ!Ò
À8ª/?ˆ¬À9ö¨y0m†@ )±`_¼(@$,!Æú%?ÒÂI;2[?ț:)Âq@Øm.׃à?ö­Œj1!?âÏàèãƒÈ¿áb×ÖK¿ç…¡êöÙ¿æ/¬*•ÕÀ¿ë¬] l‡¿Þ&«»Z3¨UNASNone3FGL J1632.4-4820$?Âï壜;?ų»<½4?ëD—ü1?ų»<½5?Ð[%¦ŒÅ?ÑáhƒZÏ£?çÒmp¬¹ž?ÑáhƒZÏ£?Ҋ=•¤qQ?¶8có~µ?æºá5-ÇX?¶8có~µ?¥_ݪý1h?–pÖ¾‰B¦?îª%P,é?–pÖ¾‰B¦4FGL J1631.7-2319c¿ïÆ˓<í@0²Ž´cI{À9éŽuy)À;_ŸÐê@ͦ;2±@"î¿eÛý?ՔžÝü ?çSfåg1@
ÈÕ[ç‡c?ÿ"˜‹Q­G?ïõûg¿,¿á¿Ú@RÖg¿ë{τ7¿é¡P°¼¿äV 7˜s¿ïõr¾
—BUNASNone2FGL J1632.6-2328c ?áZ•4òL?ОôÒ†Ä ?ÝKöՖf?ОôÒ†Ä ?Ð9›qnW?Ϲ,ûÍÐâ?çã2tÇHÔ?Ϲ,ûÍÐã?ßL´c[Ù?¹Ç΃ì?àY¥öÎR?¹Ç΃ì?Àq%è)r´?²-Owmµå?ë㶅õ£R?²-Owmµå4FGL J1631.8+4144¿ïÿÿDƒÈy@EÛLÂPrÀ;zWûi˜JÀ<êîê3@!xáî'Ô?ûg?>Ú0c?Ð$a1s@?µO%,4fd?èË.Ò{bw@PHµP"R?ïö]¿Î¸¿éµyÿ ^°¿çëWÒNí?±·K†;B÷¿åreÊÞ¿¡°lnéÚUNASNone?ïÿ¶—b–P>þ‹}¿=?Z'Zl6'>þ‹}¿=ˆ?ïýL‡3f?VéZÒͬr?5Ÿ3ÆdÑo?VéZÒͬo?ïö×⫔?duúÌï"?RP:¨×Ș?duúÌï€?ïôë/؊?G&]Ü¢rš?V) Nëòú?G&]Ü¢r4FGL J1632.5+3839?Þ%¢Má¦@Es£]gº#À;k¯{ƒ.À<™·•-#O@–A€h@EbÅÇõÍ?Õò£@ao?ã÷&<ª«:@jÉ¢uá.?ÿÇyü›F˜?ÞýÑÒ¿ê.!EÊål?»!Œ}ãkÜ¿á‰Õx¿ïÿøsCÄ{?ï¢,_Ú[+UNASNone3FGL J1632.8+3838?ëq@;ä`ð?Àùh±âŒ°?Â:ÿn|=?Àùh±âŒ°?ã3Wƒ¥Îz?Ôé˜=8‹?ٙPø´c?Ôé˜=8‹?èRNÇÅ"f?µç­2̉?ζÄàëvc?µç­2̊?àF«œƒu*?ÀÙS©$Þ?ßr¨Æù«?ÀÙS©$Þ4FGL J1634.0-4742c¿ëlÂYø? ?áÜ\WÀ85O«8þNÀ9Õt1*Dw@y(

@Ývh<)|?Æ7d+xª?äÃf,Z@f×})÷J@Œ—Å¡_¿ì.
Ää ÿ¿ËD€7Ñ¿ÖÁ'¡…vL¿çëx‰~™c¿íÍsñidH¿ïÿXÛch…UNASNone2FGL J1634.4-4743c4?€û¿€i;Ú?¶:ÒK¶+!?ï¼þ[?¶:ÒK¶+!?€LÏêýn<?‹ì@+	µ?ï¾ÌÀT
H?‹ì@+	µ?Šuõ_v»?sÑUÈÝ?ï–+"*'%?sÑUÈá?Q$u¿˜?CZ< Ã?ï÷mÿÅ}!?CZ< Ã4FGL J1634.6-4324?éõ[¯™q@ýñ.ð®À9ã'Æf>À;,èI*}@ zËA1xž@ A`ó_ß?ÄkÝþ"…¿"«¦Â?ԕcߣi&@ØÐ,}·f?ïûvΓvj¿ÊQ§g'à¿ãÌxéö©¿âÊÆͯJÜ¿é(€‡yÜe?¾¤nò	UNASNone?íçô£b­{?²Pæú…³?°ÀZäê"+?²Pæú…³?ïÖ<vB?¡l"j,e?táÄò÷ßB?¡l"j,e?ìðSÀôþô?©wóàÍ?è?¸}aøX^?©wóàÍ?ç?¼ý?~YÃm,;'?"ÿüÌ?~YÃm,;'4FGL J1635.3-4159¿ÇÊççöï@
Ϙf"²ÐÀ9Ç DC%ïÀ:þìÁ^ځ@´°z[»¾@‰'¥R5?Õ˲[‹à?êùÄ¢0ìÝ@¸à†½õ?í(iå20?ïþ2Àœ'È¿ÚFUú³dò¿ì†úÆ[¯¿åÄd]øƒµ¿ïþÒn¥Ð?ŒÑt§FÖSUNASNone?å'Q™BÎÙ?Ô'h¨SŸ?Ôû\ÍzbN?Ô'h¨SŸ?Êáªð|?ÒZãã?é{G•Càü?ÒZãã?Ù®H»ºÙ¿?´ÒiJÙ]ë?ã(Û¢""!?´ÒiJÙ]ë?_tï§uÐI?Pt½Zhƒ?ïðEˆ,E?Pt½Zhƒ4FGL J1635.3+4258?¸ ~˜_ç@E;Ÿ<pÊÀ;VzKöx˜À=WÃ5tV@©Iu¿Ê±?ý1ʘ?&†?Ñ:"Yd?Þ²¾äV×'@©äðl@
¨ˆ±>üÀ?ï 1-Ÿu|¿Ðl¸þæ¿Ô[ÉàhÚ¿ÞaŽºú½¿ïÿÒ³–šâ?ɀ:MèUNASNone3FGL J1635.3+4257?ïٟQä‰F?x°;'¥X^?s0W
»]«?x°;'¥X]?ïòjp¡Æv?v:®F`?[+¼sâ?v:®F_?ék-ªá{Æ?³d}G—*?ÊSITzé?³d}G—+?ïMzø¸{‡?O¦»Aîx?–P èð?O¦»Aîw4FGL J1635.4-3249¿æ"zBBÇ_@#±vû	 À9ç$Ã-èÀ;²F;…è@+hÌÅ@è¡ß¹8›?²¸yƒ¤?Îɹ‡uª§@§æ;2Ûõ@ür׸ä?ïÿÆ>"8¬?±é""xi¿åHpSO2¿æބ 
Q!¿éMd6á=¿ïüNÀ,€gUNASNone?ÑäÏ~P¸?ÇÚՈ4Ȩ?ç
˜rÀפ?ÇÚՈ4Ȩ?Òí º:Vþ?ÏwnÓgêd?æ‰o¢âԀ?ÏwnÓgêd?Ö ê"bþ?¶8²›qž?äïñŠ¶N'?¶8²›q?Ս"ŸFþ‰?±Äî½²ò?å95°\€º?±Äî½²ò4FGL J1636.9-4710c¿ÓTÁîV"? š&	ÔëÀ7˜ÜïY¿À9IeVÏ@6ë¤~O@‹jËG?ÀƇ8n—?ϵãfÂ+ß@qIáËa"@áIÈ î?Ñ~Ç[HÐÿ¿ÙÏUàW¿ßgçšÙ_­¿éb—oîM¿îàWÄ4?§i™v´UNASNone3FGL J1636.2-4709c4?vØùt,áü?§Ü®U…×l?ïÒN
¦;?§Ü®U…×k?'ÖLHSí¯?¢^R"K?ïqM½`'?¢^R"K?•¨Y†Ëh?F°Ö–4?ïR½3ɤ¿?F°Ö–2?gùŒ7S‰ý?\½Ã{y?ïèsȬv?\½Ã{x4FGL J1637.3-6325?¸Îöï
WíÀ%«ËÉdcÀ:¦°ÞY½À<!<(F@ý'_d@@@¡°¿P?ÒJ¢e›?Òò=ºË˜@ëó{??û0¬%~é¿ìîX}šŠ…?ï°*À¿ãOøØ¿â†ðY|s¿ïÿ']<9¿ïÀöÕ´ÒÛUNASNone?îå	Y`º?¤/Qûïj8?¡¯jiÿ4e?¤/Qûïj8?ëöïíÞ{‰?Æ–âø'Ü?À$@H†Ú?Æ–âø'Ü?é:ÓvÕG0?°
`tçä¼?˲$ªã=?°
`tçä¼?å¾ð­{ü?·0ç+‡ÿÏ?ԃÚ¥	?·0ç+‡ÿÐ4FGL J1637.5+3005?ï%¥\W@Dd| À:ãi:V=#À<‡CrE˜@ùrŸ.ÙÝ@~³¾"æ?ÆÕKÚt?ˆ ×üUÑn?¿Øš Õ£
@ÈYÖ5+[?ïü—`uÖ¿èNƱ¿åo—Òïü}¿è‰/žÔ¿ïö(°ù1°¿ßÚ{v˜ã'UNASNone?ïï<Êú?m<²œÖq¸?`Ãpÿ5R?m<²œÖq¶?ï†$—x~?¡fxS+W?Žvߚ!à"?¡fxS+W?€}H}?†à¨öø?Žßßà­à"?†à¨öø?ïB`ÌÔ?‡$P¿[¨¾?—³æpåy?‡$P¿[¨¾4FGL J1638.1-4641c?Æò}ûFš?Ê¢œâú5¼À9·ÛàfÅÀ;`®­ýÔ­@ §è½@G'Ñ(| ?Ö©Q2!»<?ïÕÿ™'Ú@ò¶ä-;¢@&½cÎ0¥¿ïõ~̹­?ì!S6Þ¹^¿wõÚã¿äúf¼Í{¿êï…>BÛÈ¿ïÿåþÌúUNASNone8?´óö›Õ?¸jú]ÞV?í|g‰,…?¸jú]ÞU?›²T‡£Z?³Ð­T»ý›?ï"o][Âå?³Ð­T»ý›?דë{ a}?¸x¦:[ÂH?ä6
B/ÏB?¸x¦:[ÂH?°ïù?¡eDHò§ï?íü¢@ßÝ?¡eDHò§ï4FGL J1639.0-2727?çÍgÛ}¤@)"¨ŸÆÚEÀ9ÜZ°O¾"À;¹¶à…@Y¤¼e@컚ua¬?ÃWq–ë?Áûÿ)ì7¡?üÖ$ê›í?ý['l×CÉ?ÏòpËD7¿â:7žÒ¾~¿æµŒt)¿á›>¤€¿ë¬`Eºõ¿ïÿÿ>¹úUNASNone?êJï*Œ'‰?Àû
£
ÓÓ?ÆÔCUÏaÙ?Àû
£
ÓÓ?çD	¿b3?ÍàÕ°ó•?Ñwíø;›?ÍàÕ°ó•?êÂûˆhUR?²K÷L›Œ—?ÄôÞ^ª¸?²K÷L›Œ—?çç̞¦Nò?«ú>X|Û?Ð0f³b?«ú>X|Û4FGL J1639.2-5638¿èrÜ÷þqÀ+äøé‹À9ñ¿ä†ý¶À;¥0°¡óÛ@sYùñs@ÝڋÒ0º?Ê÷8[;:?áÉø;æ`@:k
•ù@n‡/×?ïޝåX´Í¿ÝYßð@¿éÕá"oA¿ïýð@o\¿æ)f–7Š¿ê°ßьO.UNASNone?äÌ}Ö{v?Ïgv^?ÖgS	É?Ïgv^?̨b²€?λpáiR?èÕçSü?λpáiP?ÜòÜå\ø?¿¦ÑB<'?ᆑõ
Q"?¿¦ÑB<'?¶l—is²?¥Ë"ÕÊmÆ?í2~щ?¥Ë"ÕÊmÇ4FGL J1639.2-0946?à¡%Uç.@7¡Â # –À:òþUÀ<åê«%@ òæ0v@°nºÈ¾J?ăùdo¿¦|c /Ø,?åKÕ@Ž»o?ߕ<¯« L¿ïí	î–K0?ïP3ôú€¿·Ux­eÔE¿ë¨F`®_¿án•Š¯œ?ÔÉÞZ鰈UNASNone?ï‹èÞW'+?¼xÂ5uµ?Èju5?¼xÂ5uµ?ìV©½cbK?ȸháè;+?½J²äí¬?ȸháè;+?îúõO1?–Ý.ÉE‡b? ^¾`«ß?–Ý.ÉE‡a?ãžÚÆø'Ù?¿.ÇåßGý?ØÂJrÜL?¿.ÇåßGþ4FGL J1639.3-5146?Ô¤Fó}·ÉÀ
©9û¤QÀ8Z"ÀÀ;0r›þΨ@J(KK?ÿ'%hoU?´Á6þCè?ÓÁêAÞG@ Ã{®Í…@­±~'­¿³1¦–,QÿÞAMÝÙd‹¿Ö]B%iq¿á罞±†u¿ê0[²®=–¿éI˜ÐEþUNASNone3FGL J1639.4-5146?d=¯©§¬?]c¥go«©?ïëÂPVXT?]c¥go«©?€¡Ù+eX¾?Š¬¢µB:?ï½x›Rjž?Š¬¢µB;?«xé]N²?¢á'u—]'?îHqn*+?¢á'u—]"?p–àÙ\ß??^º!à~¥?ïÞÒ>MFB?^º!à~¥4FGL J1639.8-4642c?Ö<ë\35ª¿˜ÉF"'ìÀ7Ÿb¶®}À9,5Ý1žÞ@ }Ö§œ@¸TÛ#§¥?¿÷w›BF?ÂVŠüñ}@";~[O²?÷õY"š&1?½ï¯aOÊ?îØTTëꟿçue!ÂÈg¿æ/$°¹pÏ¿ë]"3¿áHΙ«UNASNone0?›Û"óiBí?º+e¨®C÷?ï!#Xdµé?º+e¨®C÷?†@QéF?"öÔú/"|?ï¥Ëöþ¸Z?"öÔú/"|?Äy ¤™®§?µª¤†Ø`??êá·ÖٔV?µª¤†Ø`??dhPîÆ?_>U¬:ƒ?ï뗯pq?_>U¬:ƒ4FGL J1640.3-4917¿ïó‡^ƱE¿üºüUP"mÀ9(اÌbDÀ:½ž¥rð@úü¹úb1@B_@Ø?À½ÃÚය?Èú(Óo@	¬Ÿ›;ZI@,òý8%?ê6'¾5Û.¿çj®YÒY¿äH$[ÿÛ¿ä«@ "€¿é ¨¡Ê?ª¿ïÿª¥Z—üUNASNone3FGL J1640.6-4917?ÓP§yWC?ȸæF§]?æW¬CT^y?ȸæF§]?åü3Qr»¬?Ó:¨]†l?Ô™]ˆ¨?Ó:¨]†k?á†$
æ?¸c(´¸?ÝÈó·ÿä3?¸c(´¸?á|ˆ±›âm?µÜcÃÕL?ÝîœÈ;'?µÜcÃÕL4FGL J1640.9-5853¿åž–@&À a«°'ÞÀ:*‰*¶ŒïÀ;Å0[žŽ@Õñµd{@Èb?ÍJ|Pª?×	üʃÒ@‡$Y{œY?ÿv"¹ªÎ?珻"–$š¿Ó¯¿uÌ4÷¿ä•"¦óõ0¿ìL<"Í¿áN3i¹Ø¿ïáü^à¶UNASNone?å
xÅw(Ó?ʋó|ôö?Õëu®Z?ʋó|ôö?ç
ë±Ë?ϊÜÆj ?ÑøÅê(œj?ϊÜÆj ?à^c<tq?»DãݧÙ?ßCÅ9‡?»DãݧÙ?㚧qUؑ?·8õ>$Bd?ØʱTNÜ?·8õ>$Bd4FGL J1641.3-2908?ïÒ28ãæ@&—PÁ¹sTÀ9}'šy"jÀ;š™sÚ@¶Ó'7@ýÉÄڐ?¿ª:P³Ì¡?Ö¹;àÖÄó@'Q~wÕ$?øpkܜù?ší"á4¿à£À9 ¿è:T¤MR¿ë³݆Xt¿ïÿpž"ÀI¿ïóÛ._"UNASNone?¾º[+^e?¾MÔ´Zm?ì<¨´š"3?¾MÔ´Zm?°d"Õà?À–"à8ƒ9?íþ"mŽED?À–"à8ƒ9?Ö0ÉÄöâ¢?·+ià5N'?äç›"Ž¯?·+ià5N'?•Z¾$3›?€}£Y]'w?ïU*ߦc?€}£Y]'x4FGL J1641.5+2017?âü8­Ë1b@Bª\=îxÀ;ÃcTc.¤À<ÇÉ"a:@#gß?ùiþ†ƒ<`?Ë*'Wގ¿£à­Õ:Úq?ÚÃE¤ú˹?ü¡ô;ђY¿×Ɉ'N?è{½`H?4¿Ùu
ƒ'šr¿ÚÅéï'î¿Ùn¾ú|2¿Ç]ŠÊžÊ0UNASNone?ïûö:ìÒ)?;Ó®Ú«f?@'L·Zº?;Ó®Ú«`?ïö>DÄÂþ?Ym†ö´?Sƒvvzô?Ym†öµ?ïînÍ,7?exy4%Š?a'2ÓÈúh?exy4%|?ï•xŽØV?Ú¾î2ýC?Š¡ÜxÉêœ?Ú¾î2ýB4FGL J1642.1-5128¿Å^244þ•À¨…·d†À9¼i"ïÀ:Ý(8-n@"v4åç@_­)™V~?ÒÊ"Ýtæ?àƂ@³½@e¼¦äÜ?ôÇ]_Áq¿ÕþŸb†\ü?íìk΅3±¿èIˆÇì=¿íX›7(‹:¿íÅý¥²­¿ïŠÐsJzxUNASNone?Ø´Šê?Óî‰âjC?ã¥ò:Šõö?Óî‰âjC?×,ò A?Õ+ó>"‡"?äu醯ßx?Õ+ó>"‡"?Ò(øˆXÏÍ?´HN'$ç?æ냻Ә?´HN'$æ?xQxžFê?g¡;èÀX>?ïÏ]Ãr+?g¡;èÀX<4FGL J1643.1+1436?åâŽmUY•@AuY_í¦aÀ:ÇÌW\À<8Íl.ýD@ßÿ|Øï@;ßY—K?ъ<6\?Êæc¡ºû>?õ¶¥ÉRÄÉ?ðûpú,?ïdH•:¿ç~(kBn¿ç$›?áíE¿æ "@º¿ïÿk*M±?ïú}¹©"UNASNone?ïÁrąþX?Œš
;Î>Ã?F½ÔL?Œš
;Î>Ä?êc_móËP?ÍeÂÞòê?Ær'H0Ò¿?ÍeÂÞòê?ìÛ4c?«Ïú¨«?¿™&\翅?«Ïú¨«Ž?æ=دLh?½ñCÈÐüë?ӄOØ¡g/?½ñCÈÐüë4FGL J1643.3-3148¿Ü­³ ô3@"|/øìÀ:‹O—ZÀ<DÂ<Pg@9!­NØ*?ÿ?èh3Æ?ʓù\!éà?ۅÎÁC¬¨@‰È]ÒC.@÷é¶9¸?ïôŽýß>i¿çö#]R@•¿ÄQj‹¿ÝӇ;žÍ¿íƒ9¿ïýPÃfò}UNASNone?궹TÐ)ç?Áõô¸`?Å%¬¿X`?Áõô¸`?è0$`Z¹ð?Ð#²?)Ï?Ï?n~•D?Ð#²?)Ï?á»Ä~®?½DŒK—ãd?Ýãèˆw¤?½DŒK—ãd?æ~èýõ]?®Ë©|Ai?Ó.ÛF?®Ë©|Aj4FGL J1644.1-3055?ԛN/@#d:æ…ÛÀ:&k/#:À;žM³9ä@ÙDÿŽk@í£3vO?Î,êâúâ?ÔÉÍéØ?ó›ªà?ÿ)µ@>3—¿ï8‰ÿr¼`?ïò)}§ËŒ¿ìJG¡Õ'd¿Ý‰LûoV¿ë³_¾V'^¿ïùVbã$'UNASNone?ëŸÕƒF¤?ÂçV#¥@n?Á€«åòåo?ÂçV#¥@n?ëMßhWcI?É©ø ºm?ÂȂ^¢rÙ?É©ø ºn?è0×ÍT×%?¶º'ë¨?Ï< Ê¬£h?¶º'ë¨?ì1xG7¨?«=2î"eó?¿vt=ÆBÁ?«=2î"eó4FGL J1644.1-5009¿ïlÅ^ïrÀž"B€À9†³k¢À:ïü£T-@££Ùäbk@1n¢u
n?ÓQ§àY?ÛÐo¼@I[»èxû@SóÈF*?³?¼X‹\j?¶8ÐÁy§¿ãRAK#êÁ¿êÞÊl <¿ïñà¸<?ízVs'UNASNone3FGL J1643.6-5002?âš{‡Á'®?ÍX5–b:â?ÚËð|ú¦?ÍX5–b:â?èØÛkÔf1?Ñ%u2˜?̜'P®g;?Ñ%u2˜?á>±; b'?·|5mÿ?݂ˆ¿;²?·|5mÿ?ãRf|éûÜ?½¦'ŸÞÝ?Ù[3,I?½¦'ŸÞÝ4FGL J1644.8+1850?ìà2uÆâÒ@B
Š†×6À:¾B°Ž©À<{ˆÀ-'@Eïµ+?ý¤òÈßØB?Í[JiÑK?ÐÈ b‹l@ö¹!õN@ÊCt
¿ïÛ^g"d?饣'·Ôî¿Ñù1Øýˆ¿Îa
6u¿ênÂÀÚPC¿â—À±5—'UNASNone?îãˆÈ½ê-? Ú²ši9}?¡Çst!]7? Ú²ši9}?ï˦üù/?"Y}'n_"?z,÷ƒh¡?"Y}'n_"?ì¼T(?¦L!Í;"ª?ºÅ_C–Â?¦L!Í;"ª?휤"'<?èq}²¸ä?³ÛÞÇn?èq}²¸â4FGL J1644.9-4921¿ì/ñÏ6M%ÀL,äd™À9@4ŠKGýÀ:°Ñ®³Ý@é.¦†'@
–»˜Çã?՘L};?ç}®ˆ@•ƒgþí?ú™¨	ôËn¿ïò°Vt€Û?ïýí@
¿ê\ܤZé¿ïÿøsCÄ{?ïÿKÚÉ咿ïÿþÐñUNASNone?î(JÝ5°Ã?¿^øQb?­{R,¤óÝ?¿^øQb?áf¯ºÛ?×Jœ/‹¾?Ý2¡Æ‹ÀI?×Jœ/‹¾?݃h¦§=?¸¤æ:øã?á>K¬¬|á?¸¤æ:øã?ÇWøu\?̈́·\ýf?ê?{*â©?̈́·\ýf4FGL J1645.0+1654¿ìv븜Å@A­¸<òϖÀ;ÇvK¶¸À<s;ʱiš@á4"å@šoŊ¹,?ÏD¤_E_Ü?©ì^¤Ö?܄YÒÚ-?ÿN‹‰
«¿ÔʏZÑ\Ô¿é^`¨·CÏ¿áØa@Þ°¿â!†BNÚ¿âçÉ0`¿é$UIÞpcUNASNone?ïôEjJ0?Páh¼õí™?WuÝ+k Ó?Páh¼õí?ïúº™Éób?p7õJ¢?E˜Ø2v¿?p7õJ¢?ïÝí	¥{Ä?tö?q	{-B?tö	?ïËhÒ¬?dÛ˜¯'?zKò©é?dÛ˜¯)4FGL J1645.1-4123c¿îÃò(á¨\@ý+9i®À9ËQ•	ÖÀ;R"nmØ@ â"ÊZW@œ	€²B?Ȕ¤ý¥Ý ?ÏB¨Ã
†@‡p_
¬'?þà-,3Ë?ìÖ`^åh¥?ïâžá78¿Ü=oa·ªý¿Þ3.€›ñ¹¿êãs¢¡¿âüýKð™[UNASNone$?Ê?VÈúã?ÂѧÉÁ?é~0*MÁH?ÂѧÉÁ
?ƾ›1¯Õ?̚ûËý×ö?êPY>3"
?̚ûËý×ö?ܗ­¥ã‹É?¸õ_jð'?á´)-:?¸õ_jð'?ӑQ9e[×?·ÅÐ
8J?æ7WcMR?·ÅÐ
8J4FGL J1645.2-5218?ÁƒßoãÀs©óƒð»À9¼)DœèÀ;/Ââæ@»ÑOéL_@&t	?á » Ôv?Õ¡}]ù°[@(a´Oþ@ÍüLÂ%?ïüÒf(S¿é1ÁXÐQ¿ë¯¾¿Böu¿ãr®]Ëã¿ïòÔÔK4¿àME}¸'ƒUNASNone?äŠèhð?ÒæUUêp?ÖëÀ/Ã. ?ÒæUUêp?ä$ŠÊ–'3?ÓS­:°'K?׶êjÓ±˜?ÓS­:°'K?á'eTY?ü?¶°&ìÚN?ݱ5WM€?¶°&ìÚN?Έå?³øAgs5ò?è]Æ 9¸œ?³øAgs5ñ4FGL J1645.4-5514?æ2&œÞ¬ŸÀ*è},{‰À:¨`ÔV.À;ÇÌÒ¬	ß@HýwÞ@DÄ¥¶ÞN?Ԃ¡z¹"œ?âövÛ)@©G{¿"@Õ†å"?ïç''kþ¿ãPR]šåÊ¿æk_)[C¿ë˘_1鲿ïÿÿ" 5•?ï÷üß¶´UNASNone?í¹M\Ñ?»«è™å':?²5—eqv?»«è™å':?ã]çeaîv?ÔUigOÌ?ÙD15<#?ÔUigOÌ?àòÚKç‡N?½xt»£?ÞKh0ñd?½xt»£?à`¢QM¡?Á ÷nœ×?ß>»Á]dÁ?Á ÷nœ×4FGL J1646.5-4406?¨3(<Ù?éÀ̾µÀ8â­Yiþ¡À:PÑCT§@#úäY€@²¤}"jŽ?ȸ=³™?Ã5֟™?ü¸n;Fýë@ã[:¹9r?ïþôÒ¥Sâ¿å—ñŽM5=¿à',)S¶`¿æj*sq¿èï€@'&5¿ï딾h…ûUNASNone?ʖ֛­»K?Ë%ž¥ ¯?éZJY'-?Ë%ž¥ °?ÝYò	bÍÕ?ÔÕΌ¾nb?áSûN™?ÔÕΌ¾nb?ܑ'¾²É?½]ԃ…;?á·rl ¦œ?½]ԃ…;?Ý©Œ'õ?·ý(ïY'?á+t¹¶…q?·ý(ïY'4FGL J1646.7-2154?ïýòñþ%*@-ÑÌÙb…À:°«."À;a_–i@6ãtt@Z¹ÚÁ6?ÈjkØLˆ?ßGX"%"@3̼ܔÁ@ ŽÂ%?ïÿ¶~¬®I¿á£qõáõ¿ãY.¥.ù¿ê!ÎAÒ¿êՀ?€sƒ¿ïþP½Ý›§UNASNone?¿œY¿?ÀìúX®"?ì4ȼ?ÀìúX®"?¶¦ø¥ect?Äʊy>?í+ ëSS'?Äʊy>?út	Yª?«eik3?ë>bý©–?«eik3?£Y½}ÜVX?Ž)$˜Û»9?îÊd(":›?Ž)$˜Û»94FGL J1647.5-5724¿äñ`́pnÀ˜Á@§üÀ:
·­€×+À;­ŽŸj"ó@¡Öiƒ§?@*~áS?Èz€ú'V?À¾ß8à^?õu°Ðî?ô¹#ØL\Ð?ïûÅs<7¿¿âc'·Ôî¿çº‹·XÇA¿ìõËß	¿¹HÄiüÉ¿ïú¤£|UNASNone?ï`⚥Õ×?žã™±HáÆ?"㬫EE?žã™±HáÅ?íÕ¬g&°?¼K.×®³?±RœÆÏ2u?¼K.×®³?ì½Èà+á?¥é	ë•œ?º¸ÿF ý?¥é	ë•œ?è×釰?ºY(£è8[?Ì Yãã™??ºY(£è8[4FGL J1648.1-1547¿îy¹6Ub@2Y"9ÞHÀ:'÷†®À< aïß Œ@"tX€Ÿ¢?ûíÄÉÉN?ÄQÚþ"ÄC?¢ÎéõÒ?á#œ½:ˆ'@J†áÛþ¿åµv9B@í?ïý
q؊p?Ô÷dÛ¡Ò¿àä#á0±ú¿ÑWÊ¡ú;E¿Õšü›¤ÌUNASNone?ï÷üKš|R?MKñ'‹ø›?PhËZà?MKñ'‹ø"?ïú0ªnÖ¸?d"«ßáˆ`?G=VD¥I?d"«ßáˆc?ï˪A±š?|@x®ÆÌ?zuªß'3P?|@x®ÆÄ?ï¹ìö8v?tÞ3Å
ó?"Âqâ}2?tÞ3Å
ô4FGL J1648.7+4834?í9Ф€V@CúúaZëÀ;mÔZ_ÇçÀ<Õί%@)K'Mð¤@Y{2¦E?Ӟì>Ø
?ÁñÞªïj?ò^/`?Û¸?þüE2º‰?ë{¥BDH.?çaR*o?S¿é!³äžzª¿©š«½]™
¿ç`{~¿ïþÜÇÔUNASNone?ïÚÎ_oÎ!?vPiÿUí)?r˜ÐHï…?vPiÿUí)?ï¹¹$*¬Ï?˜}Wúdއ?'¶õTÌq?˜}Wúdއ?ï£ÙÜ?…?Ì­J?‡9	¾zÈß?…?Ì­I?î ^¥€r?"〷iç‰?¥þ:§øå?"〷iç‰4FGL J1649.2-4513c?á¢F·xkÚ¿Ò¯¹Á'@âÀ8!:жfYÀ9'˜³ÀŒM@šô¥A@ÍãÉª?ÉS–€	¥›?×D¾uñô¥@úúr!…Œ?ô÷öO½¿æÊUŽ§Î?î‰IõíW‡¿äwv#rËÏ¿ì
"¸aþ¿ë*e~ßÙð¿ïÿø]Ê5™UNASNone1FGL J1649.3-4501c8?Ór%vúíå?Ûځ\™È?æFíD'‰?Ûځ\™É?"âv†½Á˜?©ñfô¬·ü?ïXìKÊô?©ñfô¬·ü?°uy¹÷òh?¦Ú¶B'‹·?íñPÈÁ²?¦Ú¶B'‹µ?DÉ)˜#<?8'®£ÙB?ïú͵º™ø?8'®£ÙB4FGL J1649.3-4441?ÆYgpl?¡Uûà
Â&À8š³zoÔÀ:6¥Nفç@xF(XcÄ@'I†\?ÄƞµbLü?ÛÒF‰QLú@Þ¶¿DN?ñ#3¾ÉSñ?ï$'¯ÀM¿ÓÁþ\緊¿ÝF1\ïDF¿ä8Ÿž–Xœ¿ìŸÖjÛ@¿ç,ÉVö†ÚUNASNone3FGL J1650.0-4438c?ˆn©Šã?¹B‡¨å?ïŸï'EYÕ?¹B‡¨å?Œ¾i˜û?—
Òîs‰?ïYœô?—
Òîs‰?‹‰xhÁƒü?vN'¥±$¢?ï'Ú\ùð?vN'¥±$ª?HàU}ÛÑ?4MëÚA?ïùÇꠉ?4MëÚA4FGL J1650.9-4420c¿ÒlbÈkC??£Ú"1`ÔÀ8W-À-À9™™ãktÃ@A0êX£Û@ª¢]yÑ?ÍZ@ãÉ?Ö®F#û²¾@"gÁLf@.Š:ÖëŠ?ï÷õoƒEš¿á^ÛÝáÈ¿â·[ÐKÝ¿è°é¬×d¿ïÿ{@>Ç?ïŽXÐàÙUNASNone<?ã¦Ó‰ú?Ù1/ÛçÒ?زXíÄÒ?Ù1/ÛçÒ?Μúµlú¨?Ò~(XSg"?èXÁR¤ÁV?Ò~(XSg"?º	¿JñÂÁ?¥âbõÌæ1?ì¾È¡Ç¨?¥âbõÌæ1?"~Á³3ý°?‰ó¥hb?ï\	òf`?‰ó¥ha4FGL J1651.1-5848¿ïó&Ž¥À"Op\‰À:lm¥À<Lï'Êr@eÂõ]¨@`¿B Ž€?ЬbÉù´?æYYø™Ú@l¯c/zA?ý‰oG‹"Ù?é(j¢‹/ɿޘüŸ£I¿à|·áƒ=7¿ïÝEö"V;¿ïøï4Ö¡b¿ëwž!"£‹UNASNone?Ôq_áô¢?ÎËoÔ¼ /?åÇP}°?ÎËoÔ¼ /?ÂK§àr'{?É ZJ3?ëmãv"?É ZJ3?É@¸™:"?®{¿Ûäű?é¯ÑÙ¾±w?®{¿Ûäų?£º Ipá?ŒsÖtÁ?îÄ^Eûhò?ŒsÖtÁ4FGL J1651.7-7241¿ÎõøáÎÎÀ1§õûmÊÀ;–÷ÎVòÀ<·•XÂ8õ@!MþºÞ?ÿöÊ,œ‡?Ë9\˜q‰¿~6¼ïMð?µW"ðbS?ñå_?ք²?îvŠÖˆ7r¿âì½B–'Ÿ¿ÜÄр»§6¿äM²À²W¿áf—éJ¿Ó®,ƒk¯ÑUNASNone?ïûØ~ZZ?F=(˜Ê?Aˆž–"í?F=(˜Ê ?ï¦í¨séÆ?üG±ˆ?ª?†D•ãŽ?üG±ˆ?ª?ïÜ·
ßË?s.Õ«(?qý$z×?s.Õ«(	?ï§É}¯"?†ñ»ËX'?ŸKÐJÉ?†ñ»ËX'4FGL J1651.7-4359¿ã-íÝ¿-í?ÃsÖuB!À8Él4Á
À:?u –
@†«×‰¿1@÷n¾ú|3?̂®›‰]â?ãD:AšT*@³Bؤ@8…a8ª?ïü7ž|ØC¿×)íÍ:¿Öª9DDR•¿æ%Ž?w4¿îrg'Ñ`¿ïÿšÜ|UNASNone?w ™¹¸ N?¡'ï"=A?ïѾ̌¿?¡'ï"=A?ˆL2;"2?—"-€n6]?ïžÏ7¯¾?—"-€n6]? ÇJ›;SK?'Ö¶¢'ºü?îó‹VLJË?'Ö¶¢'ºþ?eõ=,î5?Ro•™?ïê
ÂÓþ?Ro•™4FGL J1652.2-4633e?ׁÖú¿ø¤ˆxßæÀ6ÿÓÚÞˆÀ:4
*%mx@!?%Ó¤,p?þ»Q•	Ö?žBSŒšÉ?˜€k˜¬p?øþiâò¨ÿ?û~"æ+˜Š?É¡î&ä›K¿Ñ(›@¸­¿Þ•ƒÑF¿ÜIøœ‰c¿á–2§9¿Ûdÿ§j"UNASNone3FGL J1650.3-4600?äØ¢ãq¦?ÎĔ¿nÖ?ÖNº9ܶ?ÎĔ¿nÕ?Ý}˜õ•?ØÓW
ïö?áA3…t5B?ØÓW
ïö?åU*9cé?»¿"""ÿŒ?ÕUÝ«8-?»¿"""ÿŒ?ÎJH
ý?À?ò/»æ?èmmü€¼;?À?ò/»æ4FGL J1652.2-4516?҃a^þg¿ç—MYO&¯À8¶lCõùÀ:GHÕ[ç‡@Ø èØÇ@¯ð£kªs?ƏêÄ.˜š?אջ2ño@'ö@c^@Ç&)àN4¿ë.ñºÂß
?Ɓkdýێ¿á)à¾ò·¿éA 'oÿl¿ìàD]ýâ¿ïû.¡UÑUNASNone?r³"ä`?p)ú!õ?ïژÖ7ïé?p)ú!õ?¨¢Œ‹Ût'?¸'¨g†?îu×7BH¶?¸'¨g†?šۊþ©R?ˆD°ÜÔŠ?ï/‰#¨
¶?ˆD°ÜÔˆ? ^3µá͍?ŽB6–?îúÄ¡ã'?ŽB6–4FGL J1653.0+3640¿ïùÀÜ»@CW‹'¡¡À;¦±RFÀ<ÿ>Dß-"@Á¼.™ñX?ïö¶À›æü?àã¦Î5'™?ïöÌR֒@Šc0Q¤@~¼èS;¿åf3:¿ïo¿ì©õ÷¼e¿´3'J댿Ç–ý]
w¿ïüÙ¿úVs¿ïð²…"êUNASNone?ïdgeÉR,?•–ÞòÍ?"sFÕºˆ?•–ÞòÍ?ïÀ,|G8?ž4‹0,ôµ?éÁÜyãÓ?ž4‹0,ôµ?í-ðS m?£­ÖœçDï?¶½büš?£­ÖœçDï?íS;.Îî?«½²zÂ†?µgv&‰ˆ'?«½²zÂ†4FGL J1653.2-4349¿éØ©HogÓ?­‹ÛàùïÀ7œƒujæ(À9Žß‰gó.@@éTA÷@=¼>	P?¹{'G•Á?Ҁ¿®Xë@´û'Ã@æb I?ïþ'ÍzÈ?ãm¬átú~¿å—˜mI¯v¿çךÈÙ"¿ì'†!퐒¿ïÿ踻ÐUNASNone3FGL J1652.8-4351?´=«Æ?'?Ð »ËéÀÁ?íxJ‡8{?Ð »ËéÀÁ?s$6–1T?{CIcÖù,?ïÙ﷒Ӟ?{CIcÖù,?¡é© u?•{ªÚÉ&|?îán%oõù?•{ªÚÉ&|? »q,"~é?%ÉÕau?ïþôHí=Ø?%ÉÕau4FGL J1654.2-4907c?µÒ	úOwoÀe¦$ÂW(À9ŽX«'ÀbÀ;8òòÑCT@ÉÅjØ»î@ˆ¸»Ð`?Ç>ž¡@?Ä÷£‡?û˜…+•°@ !ÂG³¿çíeÿ8Yä¿èÛ­À˜$¿ç]Å]l¡¿ã¿FÒLhŽ¿ëe#ÀÏhˆ¿á¬åÁX¨UNASNone3FGL J1654.3-4907"?îå ĺì?£hç¥þ3$?¡¥ÿ³´QA?£hç¥þ3%?ïÄ}8AB? ÎŽô' ¥?}Ácß|_"? ÎŽô' ¥?쥍%´¡+?«ËO$œzà?ºÓ–ÒZö¯?«ËO$œzá?ï)Dת$Q?‡ä6Ð¢ä?š×e
»uî?‡ä6Ð¢â4FGL J1654.5-5509?ïÛ¦ž÷ÍÀòFà!qÀ:6ž«QRÀ;˜14@î—\R'G@Ž÷!4-.?ÔU#}³Š?îÒ/w¼Ð@å?À	oë@ĆD}2†¿ßÇ7a–
¿ÙVÁãd¾Æ¿îˆ™A/R¿Ø8ÄA¸Ý¿î?²{è¯?äÝC!½¿êUNASNone?Ö¯âEæ?ÐD3ûú(?ä¨p|ŽÝ?ÐD3ûú(?à6Oq}ƒ?Ö	Cíf°?ߓaùú?Ö	Cíf°?Ú´x^·*?¸™{NÁE¤?â¥ÃФj¾?¸™{NÁE¤?ËÈ4¹ÓŽ?¹‰ÿ秄??é:Mòы?¹‰ÿ秄>4FGL J1655.5-4737e?ïj"êî#°À@xw
À8Ý/n'"šÀ:ö´°¨ª@ €üU¦z©@¬ŒUÜ?¸.ðƒ`G>?'
ÛéË5?ÝüÙ·–Û@|²>¬
:?êؕ›^–¿×þí›ÏSæ¿éÖt`¿à¦"Àä¿Ý@€Cdô¿ä2Wk!UNASNone3FGL J1655.5-4748?ï?¥3F?˜ŒNFVTé?˜\™ŽWb?˜ŒNFVTé?ïÚí×/ùò?DE5j:G?r‰h×?DE5j:G?í?0¿'ª5?§É؆èÙ?¶zj®T?§É؆èÙ?îMòèp?–¥<‰a?«.àÑxþ¢?–¥<‰a4FGL J1655.7-2411?뇚<v@'ºYÀe¶=À:mˆXÿvÀ;áÐ>qT×@†+<™¹O@GE‹$Œ?ÒÌÌ¡Ù¯?Ñ}	@¢C@kõQPT¬?ñÙ5©Eµ?ïþ;9'ò?©2­ý(à¿éYe5
ÿ¿Ø—9¢¸ý¿ïÿë""i·?ïúY,ÁÿêUNASNone?î?H˜ß?³éÿ{£?¬vr>Z?³éÿ{£?ã¡·¥ú?ÔÒ/
e(?Ùïþ¼´	?ÔÒ/
e(?æÂ|ñ¥5?´"×5‰œ:?ÓÎ{µ–?´"×5‰œ:?ÜÒò•Á‡?À(>fœÜà?ᖆ¹5<?À(>fœÜà4FGL J1655.9-3940?ï0úÀÚ#@@®I#`À9oe5
ÿÀ;
w?Ò}ç@Dl›ßš@ۉC
@Ì?Í58[' N?Ԟ$c½ù@%XdE#ö?ûqo´Bè2¿ßÒËÿÈLµ?輸dÉ®4?ÓS]Æ.οæ7ûþé¿ç®¤"‰—Ä¿çºßr#UNASNone?Ï®êº[r:?Ê!Î+
ß?èEQi#r?Ê!Î+
ß?ÉAvΠ?Ðy}â/±¬?鯹9bLX?Ðy}â/±¬?Ú¢yf#?»aÜ)Ú?âü®øÃLï?»aÜ)Û?Çò:<'\Î?´ÍIîÌ?êqpö(Í?´ÍIîÌ4FGL J1655.9-3101??û†ø@šºŸ¹À9óëƍ«À;•ËWÇ@Ë…$@22'3K‡?Êáž@zµ?Òa]¿îî@YP%²A0@ûÅÜ¿ì]ä·¥?ï¹ý‡»¢¿æ!;¹êqù¿çlÁÊ:K¿é|0¿ïø0þ¥ŒíUNASNone?Þ€Ö*Ô7?ÌÃÎuÀS?àý?"ê•ã?ÌÃÎuÀS?àÕB.Àt?Óaíc¶€?ÞU{¢È?Óaíc¶€?ڛŸ=(m?¸q‰Â"V?â²0akóK?¸q‰Â"V?Ý{f‰Ã…C?»ùŸü?áBL»=^?»ùŸü4FGL J1656.4-0410¿çÎg­Ù±3@7.¡ ÏÀ:µ¼åÎüÀ<Š
RiY`@c
ÔoX}?þÛ£"Ń?Ì­3ªQx?ä) öÍ1@X§ç:6]@+C&E?ïÿ0,µÿ¿ç9Ù	ññJ¿œ9ÄØó²Ñ¿âž€ô‡%ú¿ëS—tü+¿ïü½àö¥cUNASNone?Ý®÷yޞ?̵&Ώ?á("Cv°?̵&Ώ?È°\MôÖÏ?Îä¦9Dmp?éÓèì'ÊM?Îä¦9Dmq?É,ú€O'q?±á£ÿ[¢?é´Á_ì6$?±á£ÿ[¢?Ð%C={€C?°H
ÄIi"?çí^aB?ß?°H
ÄIi"4FGL J1656.5-2733¿ïÿúÉEL@#Zï
å6PÀ:ŽP±É;HÀ<pSó.@ªvºœs"@kXZ4?ÍOʘ•Â?éäjþ{›'@4,ºËC@·dÒ<£I?ïÿ0ýñˆ¿è‡¤Ú?|¿³çÆÎ0$5¿ç¬—7¿‰î¿ïÿàŽ¾¿ï±g¸ÎéUNASNone?ÍÞ<ô?Ðco»p?è½9?ˆpÄ?Ðco»p?"›½ÀÀhG?©¨ÂÓ;Ð?ï["ùü½?©¨ÂÓ;Ð
?Ãå@Ÿ£!?®Yú/³Ì+?ë¯Ø—7?®Yú/³Ì*?'qf¦]Ñ^?{ߦOp ³?ïttÊÍv?{ߦOp ²4FGL J1656.9-4814?ëÌÞv™÷À	½nŠø'À9Ã;òõU'À;[;¸Ìe@UM–
îÆ@vßîÁ?Ö;Y½‹'C?ïNÀøƒ3ý@	 Vßà¥È@‹~M㸢¿ë}	@¢C¿ËßýV,‡r¿ç%IÑiò¿éŸ}ß(ïã¿â+úú݁P¿ïò¾UNASNone?áªwaç›w?Î4{¹‹É,?Ü«<0É?Î4{¹‹É,?äY9êµ°¨?ÔO¡®s?×MŒ*"ž°?ÔO¡®s?ßñ–?¸¶xMÝÙ?à4ˆ¬)|?¸¶xMÝÙ?Ò¹é˜Ó®®?¼CV®&š?æ£3–(©?¼CV®&š4FGL J1656.9-5717?ǾHopLñÀ!¤Œ?>qÀ:¬TƒåÓ.À<+óV¤Q"@=lè5³ì@ij­?ÑAǀ\±²?âȘ?|l¸@,ûõ@þè'¯q¿ï¾´ -œñ?ïï* ­Ò¿âî1× ì¿éHÂ:¢"¿ìŽöþN¤ÿ¿ïÿ¦¶tFUNASNone?ÙÅáUlì?Îà<•K7ã?ãUI‰ö?Îà<•K7ã?âÅO•®?ҟ™³/¼?Úu`ÕÄz¥?ҟ™³/¼?ԀâH¨3Õ?À¹ó´lɵ?忎۫æ?À¹ó´lɵ?à€b{D?¸F"åò'?ßÚÿ;ï	y?¸F"åò(4FGL J1657.3-6232?èç"oMdtÀ(+{®ÍÀ:jª|?ìÀ;Ódύqm@^BT8fy@œ÷_GŽ4?Ê{mI.!?¶XYÞBÀð?êÂä`è">@•¤"^¥¿ïüÏ(ǟf?Ödü¿â	€²B¿æ™Y_ç¿éßv½Ì~É¿ë{j=‹|UNASNone?ï^M
\›"?"b"ÂOW'?"6^´lw?"b"ÂOW&?ï§à¨=Î?ž(&·tR®?†Õðœ¬?ž(&·tR®?ìi»—*Ÿ?§›ÞDï?¼²#Gþ«
?§›ÞDï?î£ÓèMú?"»]Â7|ÿ?¥ÂÁ{#ÄR?"»]Â7|ÿ4FGL J1657.4-3917c?îÿ°­èÜ@TÔ#&vÀ:_©³ÃÀ;ŽÚLè@Ç)_Iç€@±'!ûÓK?Ð
CàT"?á¡b§K3@	· QºÞ?úÖ=3'(·?ïùh6J>连à7|‡Ôº¿âYl¸K¿åßbцoñ¿æÃ^)+¿ïÞ´ -œñUNASNone3FGL J1656.9-3919c8?Ù"êú'ò!?̶õ}T?ãnŠ'¶†ï?̶õ}T?É5´ç5d?Ð'ÂVaß?鲒Æ:r¦?Ð'ÂVaß?Úm$€m?µ–™ÿ¸·)?âÉm¿Ézt?µ–™ÿ¸·)?½ޒtÃV? £ÕaR\ ?ì]¤-±g–? £ÕaR\¡4FGL J1657.7-4656c?ê¢
c6ÒÀ&"»À9$¯öÓ0"À:̨¡tYn@X=EZÓ
@ÿb›ÖŠ¼?Å3{''PÓ?ÀG/~ó¦?þÙ&ýšÊò?üÀ¤ ]Øù?ïß:Þ"_¦?ê÷Û8 Z~¿Ù™»þHoÛ¿çWšPx¾X¿ßÑÃ×/Ò¿ì*© öUNASNone3FGL J1657.6-4653 ?ã¿%aŠ¹"?Î?™iöe?؁µ<êŒö?Î?™iöe?ä6JÁžì?ÓÒäT0[?דõj|Â+?ÓÒäT0[?äå=çIHì?Â	+	‡º?Ö5"1mn(?Â	+	‡º?ÕÖmsEã?¼‹D+¤Õ?åuÉF]
?¼‹D+¤Õ4FGL J1657.7-4520¿ÑRP^¥¿øsÓ¼«šÀ9>0vÀP¾À:´ç]7@ \oço@ÿ¾¹ä'¼?Å9ügÅ?´»1CïÃó?ìr9¾g¯<@%e/.Á´?ï	Zò"Ý¿ëݟM7Á7¿Ív߇ϿçXࡕç]¿êÂìÿr;‡¿¸Ï¾Ä¡Z-UNASNone?é©ÿ)÷Wq?Ä¥^—³×g?ÉXX"¢>?Ä¥^—³×g?ïÿÈ?¶ÄÄ:ÇI?œ@ðÓ?¶ÄÄ:ÇI?é}Ѹ2?³[ð÷‡Ñ?˚"¹7?³[ð÷‡Ñ?ì"µn=??ª(œ¢íw?¾êTþ
?ª(œ¢íw4FGL J1658.3-4637c?ä͵KOÜÀDoÞµ,À9Zgä맃À:×qºWC@ Ÿê§Ê@‹˜AªÅ;?Çð½Ø=CW?»`õ
]¶"?÷­íCdٞ?ö¦+'Ëöä¿ïþ°nÈ5?ïþ`ù?Ÿ¿èýIúÑÿÛÄQ¾Ž›¿ëüº0ƒ¿áü\§ ÃZUNASNone$?ë­6w/»Ø?¿AN;w?ÁK&#A¢?¿AN;w?ä¼ñÑu?ÕK[eßëU?ևà]ü?ÕK[eßëU?çÊ@œ¾ê?µ4Úšå?Ðk~Çô'*?µ4Úšå?Ѧ•en–O?¿xñùòã­?ç,µMH´Ø?¿xñùòã­4FGL J1658.5+4315?áè–'?@C#£ÂÀ;å§Ð"ªÀ<ý»9ýQÐ@!Ѐ2ë9Ê?ÿB0[è^#?Éq*º"º2¿¯ðZà:+º?à±&~
"@ßÀÅW†¿éeì"ÓiŸ¿ïî>ÅèW?ë	IàsÈ¥¿åMtýØÞ¿Ùd^—ºò?ʔG_ºû"UNASNone?ïüó\sB?5ôI D?8eeëü?5ôI Q?ïþER?I[‡Ø^î?.+¨:æÉ?I[‡Ø^í?ïé±õž–x?mŠ&yQI'?fN
aiˆÿ?mŠ&yQIx?ïö~Šdí?GـŠò0*?Së6%ÂÛ?GـŠò0=4FGL J1659.0-0140?Ø_Ÿ›Rz@7큾±À:»df²À;ÛVSÉ«°@6ÖS3XÈ?ý«m6d@?Ə¿P7{?Û¬D6¿@a¸¼-B?÷ÚJ><¦¤?ï ÊæB¿˜¿Ý ="(¿ÍÄüžÌ‰[¿à^ý':пïû½ü?ìôêÃùUNASNone3FGL J1659.0-0142?«Ÿü°
ö}?®Å¡Æ}jG?îF4ÿ ˜?®Å¡Æ}jG?¿!½²#Cp?Ëþ÷¯Ë?ìÈI»—'?Ëþ÷¯Ë?°`¢÷†û¢? ¬ý&Ä°?íóë¡ ‹? ¬ý&Ä°?ÀZ»*Ê?­Î.¸ô4?ëüéQ5~Í?­Î.¸ô34FGL J1659.2-1443?î°¥¢yÆt@0ÉõœÏ®ÿÀ9úú0³&3À;ڻݑ@/@ô%ø¸
"@‹Ù½v?Ȉ}£–s?Ó^lÇÔ@} >ÏI@—†¡ð*J?ïýW¿.©Œ?ÐëÂßä¿äTŒÿØ<í¿Ùª‡Þ0Ly¿ï['\¼?åF>QÊMUNASNone?ë6ýÌÃ?ÃRDÐà}?Ãã'"Ì÷?ÃRDÐà}?ë]qþx
?ËË4æ?
?Š8ŠÚ?ËË4æ?
?æ[ñ®æ¾×?²×®"úv~?ÓH¢2'S?²×®"úv}?ì57҅âx?©X[¡è¶+?¾VAkÐìC?©X[¡è¶*4FGL J1659.6+4918?ìélþbj@CpޏlðÀ;§iϧr À<ßjT1°|@"yÅï@ÿÿ«Fj?ÓZ]āNÊ?¼.)‰_?æ×
˜n÷/@œ=D:¿íèØÁ¢¢,¿åP³a@➿àz=|bQ¿àœýÒ(V¿ßå»[5ZÖ¿ïý(_D´UNASNone?ïýèÀ"A?.Ü=pŠ2È?0¹ûÝ÷úá?.Ü=pŠ2³?ïýˆo,ö?X':@-è?3¼†›ðS¶?X':@-é?ïèùö#R×?qÐ7Uõ:?g	Ü­(þ?qÐ7Uõ8?ïó™ŸQ3§?GÌ´9"/?XÌÁ]˜±?GÌ´9"'4FGL J1700.0-0122?ç@h¼?`"@7ÝxqOÎÀ:oSשÀ;Ä76Íòg@Aº£@°'w"Œ?ԗg›ñ
?ãÁ1"·ºí@
çööl@ys×=>$?æA-ô/?ä˜`‰' ¿á…²œøŸ¿ë¥<e¿íÁ¼-BXj¿ïþ/EgéUNASNone?'€Wß®÷?›i9dF<â?ïkƒýAˆ?›i9dF<â?Ça¶–$Xz?ÏDܸHŸ?ê''Zvéá?ÏDܸHŸ
?Ä!Øx`–¥?¯Ò¶¶·ÐÎ?ê÷‰áçÚW?¯Ò¶¶·ÐÎ?:^Ñ:Í?…°œQK§5?ï-	v)˜?…°œQK§54FGL J1700.2-4237c¿Ü»­ú	F¿É=4D«+À8N>X*cÀ9ñ²½W@–ë_µ@G`Æu?ǹNè›_?ÜnÛëMÁT@d öðŒÅ@ˆŒxô³q¿êâ‹`òË?ïüJ~Sm¿å-݈ܳ¿ì Ñ0à¿ïÂã>ÿ¿ïö'=¯¸ëUNASNone,? A[‰ÿÁÄ?»4G³Å$T?îûêG`ã?»4G³Å$T? :ž8'b?µë_èÍ'?îüV}‰Ý?µë_èÍ'?¨r:
µÑo?š'ø€Øô?îxÜ_T¢é?š'ø€Øó?v"›—ÝZ–?gZMBËß?ïÓºÈÐEK?gZMBËß4FGL J1700.3-4557¿²(õËý'ÀyãìëÀ9&p­FÀ:ŠšÔ,<Ÿ@ÐÁ{µØê@#Ɔa®q?ʘÜñç?πåÇFü@c›{)Q@¶•bþ'
¿å‰¡iq³¢?ï†Nc:aü¿æüÚQοæjqáÕ¿ê4{'W]µ¿ïþêÁªYÛUNASNone?Ò2ï'7¼?ș'ÕŽ¹8?ææˆ}ld"?ș'ÕŽ¹8?àÖ禶<X?Ôó\ð xó?ÞR0²"‡O?Ôó\ð xó?Ô[çãeÚj?¸½C|ñ¯r?åÒMË?¸½C|ñ¯r?Ô( 	y¶g?¾¥Üѝ?åë¯ûC$Í?¾¥ÜÑž4FGL J1700.4-2746¿î%ŸðÔ@!¼—ú](ÐÀ:C	^M"1À;¸+`ÖÚm@N'·ވ@L'Iñ?Çݏ'¯›?°›»\âÙÿ?æ{—P=Ê?úQÕøÅy?¤; :XÓ?Øß-jä%¿ëàz©"¿ßþè(¿ãƒHõ<X¿àҍÖí·ÿUNASNone?íà‡Ü<Y:?°2œ³ïr|?°ûÁ6)?°2œ³ïr|?î‡Ì?I?¾'ú†¶€#?¯~Gƒ<y?¾'ú†¶€#?ìÏ2³ÂA¤?©ÑòØn
?¹†jaíòß?©ÑòØn	?î9{ ´?™mSèoªe?¯ÜhMô¿?™mSèoªe4FGL J1700.8-5218¿ïG›qcÀßþó…õÀ9ØU)þKÀ;uÌ¥_ z@bQãÍo_@ãVg?ÏÚû#L`V?Ïud8#2@â˜E܃#@×;Ëz?ÖÊ¡¤U	r¿ë•X¢žÁ¿çn¿0,¶¿æùÄaÄ@6¿ïþùoÃz¿ÔÓ@h¥ÜUNASNone3FGL J1701.3-5216?ì#sëÏÊ ?¹G"Ñ}k†?¾ä`¡«?¹G"Ñ}k†?êíÚ<)F?ɮ̇ÐÇ^?ÄH—[–ê?ɮ̇ÐÇ^?â"FqÌçø?·=8)U?ÚÙsf0?·=8)U?èUÆdH‹?®‹é0Guú?ΨænÝӐ?®‹é0Guù4FGL J1700.8-7304¿ÄʍՎÙÀ2jázû]À:ÿȘŠ¥áÀ<w7ð1Uã@VÔ}›6@jÕ`ðà?ß{2{R[Â?à!ï^G3@vn¡žJÙ@[<'¦?ÜëÂFa
?æ÷©OBÇ¿à.Ìț¿çÐÉ{ßto¿åÕN±=û
¿ïæïÝ ,UNASNone?ïÁ¶'-P?'˜rq°W?$ìiWýÏ?'˜rq°V?ïì{aâ.?"j"–Ú?có"žѾ?"j"–Ú?íùØõ95´? ž*ò#?°18V6R]? ž*ò"?ïO"ù©?‡ ÇG{¨?ÖÀÊæ?‡ ÇG{¨4FGL J1701.3-4924?á¾}	^$À
2±-4À9Á.^¸<À;=¥."R:@JÀ¾ ·†@ Uûµ¤?ÏÊ,–?Ò,¬{ž†é@:ry\ã?þ<«tp–¿ïþÐW›È?ïý‡ŸñøU¿çÎÇ]øÛ¿å§û'Ü5ö¿ïþ'ö ?â²aFkõUNASNone3FGL J1701.1-4930?çÜþ7_~ƒ?Æ æUËc?ÐF'Aù?Æ æUËc?âh&³½l?ÔÀ%3	Ó&?Ûã/²˜…)?ÔÀ%3	Ó&?Û6ouý
?·ûîi ÷à?âdÈEy~?·ûîi ÷à?É{wMÊßU?¶õ¥|ÒF«?é¡",H+?¶õ¥|ÒF«4FGL J1701.9-4625?Á"^¡Í=À7´·,À9¨3ša?¶À:Ûd53¾s@/©Ì—Á@¥æ¼b~?Ðkj|uœd?àR=à
l@@
?:¬¤8@´™Æ»á¿ÖW}ë=P¿èÏ"Îš¿àôG/iz¿ê2þº…¢¿î?.Ö­ ¿ïSÅ¿½DÅUNASNone3FGL J1702.1-4623?·IÙÌƯí?ºëâm$G?íÄÆg*?ºëâm$G?Ù!õô©œZ?ÓÖ´·÷ØH?ão«1Ó?ÓÖ´·÷ØH?Êï셒Z?´S¾HЇâ?éDޛiy?´S¾HЇá?¦-ë¯*K+?"(70á¨?î!E
[M?"(70á¨4FGL J1702.0-3721¿æIeq!:@+xÚq3À9¦Å¿'Q§À;vy!@ûÝÜ@MÅ2¥?ËbV6mzW?Ð ´«m×t@ZÆ3¡î@ZªBß"»?ï±ï,»J¿´{ƒ"…F¿Û»âï£ç¿ã´U'¿êS±Þ3ý^¿ðUNASNone?ØÌ ÿD?ÎûÍâ7±?ã™ïÀ]ò?ÎûÍâ7±?ä Ò¾\3×?ӗM
Ýz?Ö¾ZƒG˜P?ӗM
Ýz?ދG7b,?»k út?àºx\dNé?»k úu?ç:ˆÕáá?°;·1Ó¯Ô?ÐŊîT<<?°;·1Ó¯Õ4FGL J1702.3-2525?êÍ'ŠÞ@#à#éêÀ:9êØPÀ<Ğ*"@²Wz>ý?þý@´%?È`hàê*?ÒUûŸž@à•äÙ3
?ùàçß!ä?êý"à¤ðæ¿è¬ÍT¤?ÐCCrE˜¿ÙØŒ'Á¿å³I€C‡¿ðUNASNone3FGL J1702.1-2524?îä¦_p×?£?èbÿ×?¡µŸò˜?£?èbÿ×?âåq2¸J¨?Ó³!ˆç?Ú5šj±?Ó³!ˆç?é©ô©¿?¯9+	(t4?ÉX-[…ð?¯9+	(t4?áÇŽñö
?¸8"!f\Ò?ÜqÂâì?¸8"!f\Ò4FGL J1702.5-4803?ïO±"¹¦ýÀÅS[ǦóÀ9»[>À:曶ªK™@¸HýÏ@Á`Dä5Ÿ?Ý©Ga"mÛ?ǒ&>?÷1Me
 Ò?ûæ6mÐ=¿íöÞï@5?ïõuüŸ¿ê¿Õ£5#οéJ>xᓿå¦ÿéYËM¿ê¶iLUNASNone?æ؏sç'û?ÊàÜ£ð?ÒNá0Ú
?ÊàÜ£ð?èٙº¾Ëˆ?хpøP%b?̙™ÑÝ?хpøP%b?äidLR"?µÓkÝC?×-7gZÖþ?µÓkÝD?Ö…1sI?ÁÊëþ?äõ=gF7Û?ÁÊëþ4FGL J1702.7-5655?ê(Ï|ع˜À"u?À	oëÀ8BÃEdŽÀ;EeìÃã@{¯xÓü@ÖÔ=–?¤¶Pð?Òò1ÀíE"@'ÞSó@/;Ÿheš?ïÌ
ÑyÛ¿Øm-_´›~¿å\iànj¿è¨ujhS¿í†ý )Uº¿åxYã¡$¨UNASNone3FGL J1702.8-5656?ƒ|û"7þú?¢©8 zƒ?ï²ï ?¢©8 zƒ?võÎRz!€?ƒF‡ó³Î??ïÒc[¼?ƒF‡ó³Î??µÏYƒ&?¥Á†܃p?íFϞüü?¥Á†܃o?.û/°Õ?	ò7GŠ?ïÿwfˆ&ƒ?	ò7GŠ4FGL J1703.6-2850¿ïê*
O} @¨E/‡­À:@€#À<8¸®1×@ Àåä@Ó~9Á®?ôæç€,`?؟ND0±y@=®ˆ*Ü@o¬.œ Š¿ï"ôÁ?ïU"âOÀÞ¿ÒU,«¶¨¿åÜ_ag¿ì´¡mM‹¿ïÿû-2h2UNASNone3FGL J1703.6-2850?Úþ‡ÔRe¢?ÊIU)˜ÖK?‼ÖÍ/?ÊIU)˜ÖJ?ä¿ñÍyŒ?Õ릥©é"?րeçÐ?Õ릥©é"?ħ±ÚFc?±È¾kï?êÖ‰ng>?±È¾kï?áí³@™I}?¸#ø՞
¥?Ü$™~Ím?¸#ø՞
¥4FGL J1704.8-4030?ïŒßÆ	›•?Û@¬B"£`À8yÓ3[AÀ:LèÁõÙ6@Kû+/@äÍt'y?»¸€®­?Ôñ[!ŽÆ@Œ[J©q~@y2 ?ï֘Þ2и¿Ì,gç𿛿φ\¥óD0¿ä³¼ZŽÂ¿éÚQÎ_¿ïÿÿ" 5•UNASNone?"q?×Å[Ä?°%dJÙM?ïdvAÕ"?°%dJÙM?•úÀÁ‰*L?¯Û/Ԗ?ïP)ùó¶®?¯Û/Ԗ?·˜i"ì?¨Ï3 @Å?í=ò͂?¨Ï3 @Æ?zs",øv?iªžšÒ?ï|,c^˜<?iªžšÓ4FGL J1704.9-4303¿Ñ"Ý'["¿ò'U^×%ìÀ9a@®Eù	À:‰q€Ø@ %ù	@Æo@SjZç­#?Õ¥dd®€?꺪ùš‹@2&ù'Ô@í‡@¬n?ïÊ4f?êVžrFny¿ÙÇU¿z(æ¿âuÂú»ó¿îÒ¾©HŽ¿ï¸fC*÷ûUNASNone?ÏKLi+îÃ?Èn¢"èÊ~?è-,åµO?Èn¢"èÊ~?ٍ"1Îzä?ÕÌ+ì_£¶?ã9nç?ÕÌ+ì_£¶?ßޖñ…?µ­~h¾A?à|´ô‡=?µ­~h¾@?ÇvÚçØ»?µ%\\æì?ê"IF	Ñ>?µ%\\æì4FGL J1705.1-4748?éJ¼¹³ŽÀ+†±_ˆýÀ9«8bGÀ:ä€üê¡Ê@C"~øX—@+ôË—¦?ÔÏ ´?ØôóT¡@ß	ß3Ø@õkšWÛ?ï{úýŒ³,¿æêÛuÜûï¿äXŸ›fM¿élá8"œ¿åÆ×õõ»¿ïÿÚ
¢ñ1UNASNone?äÅ_ÜDY¬?РÒÛ2Z?Öu@GwL¨?РÒÛ2Z?æ,Ù Âûò?Òz‹g0Ð?Ó¦L¾z?Òz‹g0Ð?ÝYgÅ_ ?¿íÀüÔ$?áSLP}°?¿íÀüÔ$?Ñ"ܦ'€?·àM¹z?çrµ'¬ì??·àM¹z4FGL J1705.2-3850?'þ¶¯¬«?õÌ߬£a™À:
E®_ú<À;Ë°Àý‹±@Qlut c?þ(j'TÙ?ÑYF'ÆCq?êøPV×@0šú©]@3D™âê›?îÊâa‰‡Ô¿ÏSJ˜Õy¿ÒZ-òï¡¿ß9çíºƒ¿ïó£¼2?舘TõûšUNASNone?Ò2ÇE…ûf?Éx‹tc?ææœ]=N?Éx‹tc?։³Ïnd?Ö¯)Fáé?ä»&pÈÏ?Ö¯)Fáé?Ôb‰¾|Û¦?¶Er'pá˜?åλ Á'-?¶Er'pá—?ÑĔWZ¸ì?¹ôðtPÆ?çµÔR£‹?¹ôðtPÅ4FGL J1705.4-4850?ïÀ¨Mƒâ¦ÀÌ}´'mÀ:9V"tnÀ;‹«‹3¥I@8‰ëPÆl@S|~֟´?ÖœÈù¶?æ‡ÁÕÍÒ@ìMìm@8JŸo?å',Rnaݿ∉ÁµA–¿Ú͈ßb%º¿é¹ëžŸÿ¿ð?ïÿÿÊPËUNASNone?ágBé©Bš?ÒÅÉ	!Ü?Ý1z,­zÍ?ÒÅÉ	!Ü?â!¬n?Ö	mçD\u?Û½Éñü§$?Ö	mçD\u?Ô^Í	ßæò?´Þk4'F$?åЙ{‡?´Þk4'F$?à'{õƌ?Á=K³m¡
?ÞÛÛrç?Á=K³m¡4FGL J1705.5+2907?ç9ŸõÍø@AR¤~Ïé¸À:¿5ÜZßJÀ<\m.׃à@ùpâ†@Ðfd¸ç=?Ȓõ%0'?¶V¯d1,ô?èäK8ãv\?þŒ³t·?Ùiå‡ó¿ßsd%Ä`¿êA_f¿ç	OŸz"+¿îìSE!rA¿ïì`Eºõ4UNASNone?ïnÑù^«w?'ìÊ¿S_µ?'%ÀÔ*'?'ìÊ¿S_´?ïvi–êF?ª¬Ù
?2Í"·T?ª¬Ù
?ï
÷íߨ?'‹^Uº??žAD
ý!?'‹^Uº=?íÖڃV¤?™ déÔÌÕ?±I+åK'å?™ déÔÌÔ4FGL J1706.2-4950?å0[À!üÀžÇ†;îÄÀ:ðp@üÀ;ƒ€ýÁa_@§l®)±@‡ãúû÷?ЯIĚ#W?ÞúôþD>@e‰ýDcÝ?ø
t";¿¿å\·ûeg¿ÖóI¨Pí¿ã¾V<"¿ëä ©m¿î÷Æ`!'î?ÞFžJ''UNASNone?Ȃµ˜ú?Ã=`³XQ?éßxúR™Â?Ã=`³XQ?á4ûkäiª?։îÃå§?ݖ	(7,«?։îÃå§?Ë]yD¡;?´iœçÑØ?é(¡®×±??´iœçÑØ?ÁÛMÃ҇¹?ªþÅÙÌ]?ë‰,^?ªþÅÙÌ]4FGL J1706.4-4609¿àÂk‰ÈmÀ	ÄȼœÓáÀ9¬¡´NÀ:ÜC8cõ@ !¾‡z]@åàdYEì?ÜnÖwpyæ?ÖÝqà˜Æ?ýƒ3ü†Ï?þ±ì<É¿ïô‡'YY8?ïú:þпׅì~à¿äW¬ŸZή¿ê¥cÒ7oÙ¿ÕW`NjUNASNone?Á'ÿùæÕ?À!Ȝ?뛀†J¼?À!Ȝ?å5øÓ¦ít?Óµ"º£+?ՔX²%?Óµ"º£+?×óõi<Lú?·91(›@?äKaك?·91(›@?ÐZ¢R÷Üä?»aqëPQ?çҮք?»aqëPQ4FGL J1706.4-4649c¿'›ãý,!OÀüœü$©-À9Ëû¹IÀ:ôÞW(Ü@=GöŽ½@^ú|2€†?Ö÷Ö»¸þ9?íý«w@	ízÂ=ý'?ÿ¦Tè凿ïÿ¿h`;ª?ïý­àx{<¿éðˆ=ќÀ¿ìZ¬‰`fr¿ì…;=ð?ÊÊ¢{žHUNASNone1?ÝRß3ªß?ҝùü­Õ=?áVûf*?ҝùü­Õ=?ޕvv÷?ÖOî_ =E?àµDþDþ…?ÖOî_ =E?×aßÁJµ?µÕc‹Hó›?äOrZ¥?µÕc‹Hó›?ãñø`^?^CÊØp?ïpàp<þ?^CÊØp4FGL J1706.5-4023c?잏9Ñw?͒Fiö¦À8…™1"ÎÀ:g°éAx@Xô"&@qœûMê?Ɂ©ù8:¯?ďHy]d@o¿@OÂ@*5³–?ïýFA­¿È+³1fª¿æÅ»Áã¿è(žŸ'×Þ¿ë\½جտïÿúÁҝÇUNASNone8?äq§«
á®?ӐCQ'¥‡?×°©ä<¤?ӐCQ'¥‡?Õ°%÷–Ê?ÔmžßD
é?å'øí4œ?ÔmžßD
é?ßäÞoZ^?¶ÝÀ풺#?à
ÈRûÑ?¶ÝÀ풺#?ݚ^7;¸a?½¼·!v>?á2Ðäb#Ï?½¼·!v>4FGL J1706.7-5525?â±d0ü»À!"½8SLÀ:-únƇÀ;¯2c)›@ÿwšôŽ@°\‰mÒk?îŽ|?@²£?àµë÷öF@î¯?ôÖ@^Ѭ°w­?éՌŸ
FÖ¿äÜ¥R4€:¿ëM£Œa¢²¿è!ìÿ.¥¿ÛBwî¨j¿Öº
›5¦UNASNone?àtý܉?Ò].h·Ð?ßÍæFî?Ò].h·Ð?êmŠéŠ?Î'	©…Ç?ÇúIÔ[Õ?Î'	©…Ç?áSv¨?Àyƒ¹Ä^ ?ÝÛYÃô®?Àyƒ¹Ä^ ?åö(–÷˜Û?Ãbñ~ö¡?Ô®ÒÎJ?Ãbñ~ö¡4FGL J1706.8-4540¿ê¤B~›¯ÀðîÐ,ӞÀ9
:¥"À:x3⅛¶@Òå°@Äú¦#ë˜?Êꡞ÷?ÍWåÐD&@q£EêÅÜ@5,ìG;~?>t3¿è 'w"Œ¿è<yÎ"7b¿ëZÉD'¿äÃ4½ÌÔ¯¿è
q=Yý¢UNASNone?ä:—" Y1?Ï&êdðm?׊Ð÷¿Mž?Ï&êdðm?çض̊à?Ñäíðõ4?ÐN"Èfê??Ñäíðõ4?âyàÍÑÊ?·îŒ.4?Û>d]Ðm?·îŒ.4?Û-3ýJŽH?ÀŸ3œA÷û?âifZ¸Û?ÀŸ3œA÷û4FGL J1706.8+1319¿á®wEÄË@=
ù½Æ À::¼µ'•À;ó
÷9ˆ@tŠ‡¿@˒}E¥ü?ÁnÝÃÀÄ?³jzF?À»~ãH@EÝ
$q¿ä#gC8N¿ä>Yl'à¿ì›Cót×B¿èÈΪŸ¿êb!LÖÈ¿ïðCÊZ+ÆUNASNone?ïêiz°oß?jϚ!}"?e–…O!B?jϚ!}–?ïìD˜t=¤?†¢ö‡Çk&?c»g‹Â[ò?†¢ö‡Çk%?ï-|ˆ¢¤??"þJ>Ë?šPnë«x?"þJ>Î?ïݞ-Œš?bÌ0$Ώ?q0þé9²Ñ?bÌ0$ÎŽ4FGL J1707.6-5351¿å<–¨Ï{HÀßþmXÈïÀ:dT§!A™À;ÁåN£Ò@—›±vÚþ@œ zûI?ƀ"9»¸}?ŠéÖë+)?ÈæX%?èhkêòÃ?ï´Ó³¬j¿ãSæ1!àû¿ê.‹-Æ¿ä㮀†x*¿àÒ1@ìF¿Ü¥Ûüëx‰UNASNone?ïÃ~€˜E?'dØ{½Âº?~|@¿³Ý¶?'dØ{½Âº?åßfõ?¶J.‹L6?¥W¢	®?¶J.‹L6?î¨
7ª'×?—°îÇËE?¥\…Vâƒ?—°îÇËE?éêít<º?®×á^ùS-?ÈTJ/•?®×á^ùS-4FGL J1708.2+5519¿²ˆãÙÏ2@BE"V!uÀ:ò¼~ ïÏÀ<‰
ä¹S@4,AQ"@ÁÛsX½?Á~$É
$¬¿²¿^z3͸?ðÞu†"Ú@•^XûIJ?ìñeh9¥=¿êŽÆÚ
M¿éóëÇkd¿â³@S'D¿ïÿï¤h)µ?ïÿyYˆUNASNone?ïñm`ئü?b?¦ÉÛ>†?]%>N²h?b?¦ÉÛ>'?ï¯Þ(Ñ÷?£Rf†â?"<Èu˂N?£Rf†â?ï¾ÖD®ø«?|!ªP|³?€JnÔAÕ?|!ªP|ª?ïÅè8ª–Ò?r"£AÆ?}㪴–ú?r"£AÆ4FGL J1708.8-0923?ë0réÄb@1Îû"‰µÀ9éÓbCÏÀ;tgVPn­@¨¯Ýþ£_@Æç£è`?ÏêéWòÛ)?ÎÀ|œÞ…@úälü'?ý¢™gŌ?ï;š«'"?ë†'_8u¿æ3ý}Ħä¿è:¥Ž¦¿ïü‰Þ™–¿ïÿþBe«+UNASNone3FGL J1709.4-0917?èè¤Ev?ÆÀ…¥h"?Ì]nëþ'ð?ÆÀ…¥h"?Ö<ác˜ùæ?Ñþ®òŠ·e?äáN3ƒ?Ñþ®òŠ·e?ߓjÅ*Ú?·)¤j™&?à6Jj'ü?·)¤j™&?Ë˖,Ò¬?²Óʈ÷	?é
tËTù?²Óʈ÷	4FGL J1709.4-2127¿ÇZ\Þ¿ÊÉ@%ãU>S"À;8ÿI÷š×À<ǂ4"F|@ ÝɅ¯Ô?ûT^[Õé¬?׆ncàÐ?ïò%ÀoF@ُ>Õ(?üïTa+>¿ï2QÁ"³§?ïýµ7"Ñ‹¿Ørê"ž ?Úu^<¿íAWîÔ^'¿ïýÜÚa
UNASNone?Ù»{D£Q?Ê»ÒK»œ?ã"sÂ]®X?Ê»ÒK»œ?ÃU*¦ÉTg?ÏéצàÕ?ë*µVMªå?ÏéצàÕ?ÝŽ£r•ï?¸E¢4rº?áv¸®Fµ	?¸E¢4rº?ºù6–¦9?¯ƒ†@~Ö®?ì Ù->8?¯ƒ†@~Ö®4FGL J1709.4-0328?ļ\Že¶@4ÅE¥ü~kÀ9hAK#êÁÀ;µ´+W€@˜XpÚ^@ORƒZ'ô?ºÛÅc!?¼…ùԗÇ\@tt–ªÑÐ@ÌûÎÂñ,?ïʑô‰ª8¿æÃ:aû›¿ä	z!Úh¿æFÔ©¿êIßÇü.¿ïÿ (ÿӊUNASNone3FGL J1709.5-0335?íȜy?­:<ZØaü?±»?'$7?­:<ZØaü?ährø™LÝ?чô£àéŒ?×/ÍfD?чô£àéŒ?ëôáá|?ªxٚä™?À,{äzß?ªxٚä™?çž…h+?®®zïPI*?ÑèÂõ÷/¨?®®zïPI*4FGL J1709.9-0900?ïíiÑH7É@1ÆüvÀ9þCiâÀ;­iQ;@z*¨J6…@Æpº}>ð?Êpkø̄þ?âžÏ™/çN@œ4;pïV@ìÞDïHM?ïö8 WäC¿â @|ÇÑ»¿âºJÿ'¬˜¿éUao0º¿î×nF.¸z¿ïÿýç!éUNASNone?ÈÝø¹>D?Åóœ±Ox?éȁѸ0o?Åóœ±Ox?¡"è$O
?²À.ún?Ñ?îæÁ~m»?²À.ún?Ò?Æ}a‹'0?­²? Þ?ê`§:[´?­²? Ý?£½îŠ,¦?‹ΗTâ™?îÄ!]5 ?‹ΗTâ™4FGL J1710.0+4629¿ïínýƒ6c@B/Øf€À;	|gY«mÀ<¿¹üæp@±Æáü4?ü=''N#z?׬9¯N?ÚÚÙjj&@?mƒ'˜?÷Ï'EZ?¿C¬ÁÙB–¿è¸V¿×-۝ôr¿Ý"§BÔ¿èY`Y+"¿ïø"PŒàNUNASNone3FGL J1709.9+4624?ïÀ¼y‰î?'ëí̆£w?¡Ã;ü ?'ëí̆£w?íøz Ñ?¸%Hwý³?°</¦ÿ!y?¸%Hwý³?îWôÀ??(‹
ŠC?ªŽ°³þŽÚ??(‹
ŠA?æˆÓu?²Î?²Wš?ÓÛðïÖY?²Î?²Wš4FGL J1710.1-4541¿îöÏQegÀ·'Ôà˜À9Òí˜oWÀ:Ä]ºÆ:@ ÝÒÕzp_@­D¦">?ÅáÈÇÚt«¿öå=öŸ?ß$¥Ñ¶A?ûǕ*t¿èI ]?é|×V"ŠŒ¿µIÖã§å¿é=êFZWd¿å<jIIõí¿Û+Í
dl'UNASNone?ë03ï-ú×?Â'oá2Š?Ã?0CH¢?Â'oá2Š?î·'M‹áY?¾CìæQx?¤‹'Aêu?¾CìæQx?é&å,}>¾?·Î(Gó1Ë?ËdkN?·Î(Gó1Ë?ë@-#˖?²Èj™9!j?ÂÿKûpÑ©?²Èj™9!k4FGL J1710.3-3039¿èÛ£•VÀQ@¯¸á]}ŠÀ9íŒa¢²GÀ;"\sž]N@Ž`¹~;o@Ž8¿,Ñ?Î=ÄfKä?Õ]mÄS¬z@˜:ôȔ@0…·e¿·òÅYç?å«ö"o³í?…§	Þiñû¿á¸FB"‰è¿é¶É™"{¿ïò…Ãù¿tUNASNone?õ¯ïÙ\?¼À"1±r?ë"	¨ù?¼À"1±s?×ؽfçü?ÑÕéÞÌ!Q?ä÷¡LŒ?ÑÕéÞÌ!Q?Ùÿʑd?¸É"­|ÃP?ãsø€·N?¸É"­|ÃO?ÖÓÑã…o?µF`}–Ê?ä–=H8?µF`}–Ê4FGL J1710.8+1135?åý(9b‡@;‡dº"¼À:²?d™ÝŒÀ<*.wÐ@p›ž‹@}ãZ­Ë?Ù´…-Pñ?ïÿþˆ0»Š@¾¼@ŽÉ@ÇÀv?ïíöé	:¿Üè@Ü;Ç¿îÓä¿ïÿÀ¿ù)Í?ïûJî:Ü¿ïþ@ý÷DUNASNone?ïïfïô?s·»Ÿ"ü¨?`™ôpÍ?s·»Ÿ"ü¨?îi"'›>?Á9ӄ#>Q?©g¸æL?Á9ӄ#>Q?ë=îùF~?«šR¹mØq?ÃDæø?«šR¹mØq?î <
Ô=Í?¯<òTçµ?­ü?"¼#'?¯<òTç´4FGL J1711.0-3002¿ïÜٕƒé@'Õü3ÃÀ9ç…w£¥ŒÀ<ìxc¾ì@äQ&@áf?È9ÜÛÖ}?ï@r¶ÖÁ@Å?9ѳ?ðSœà ?ïÿÿ)@k*¿â pÎI¿Ñœž|ƒ8¿êYÇòrxÿïü"Åý¥³¿ïÛÖ¿•UNASNone?´·ëm;?È]AÜÛI?ílIÒX?È]AÜÛI?üØ´h?¥¹o€x?ï¸
¼ŸÍ.?¥¹o€x?´þ<˜GÙ?¢GԂèù^?í`8l÷?¢GԂèù^>õwhöæ4Z>çuŒ¤!M¨?ïÿÕ.3>çuŒ¤!M¨4FGL J1711.4-2526?ꢖ.BQÊ@ ‹ææS†À9¾çBsBÀ;€¨AÓ	'@ž†¦!è2@©õ1?ȇiÁ9Æ ?Ìmš7NJç@MNûÖ7@ºJyJï'?ïì2ðî¿é¨/"BAÄ¿ã%DȆìï¿çÝî'ð2-¿ïÿ÷fÔJp?ïÿ!ž5_³UNASNone?먃~R6?À@÷d€±?Á]ò·ß%?À@÷d€±?éeQ÷v´?Í7öMþ©a?Êj¸!Š%/?Í7öMþ©`?䀁Ý(Ù?¶úÊs<½Æ?ÖþüE¯ÐM?¶úÊs<½Æ?ëZ¬À\á?®./õ½‹?•Lþ"y?®./õ½Š4FGL J1711.9-1922¿èsf*"à@'PoiDg8À:]^ˆK"|À<eˆEßÞ@g¥3€µó?þÆxõ?Æ6Ükü(?à{:Ôd¬@Ê~=ó?ütá0‡o?îß»‡*+M?î!ÆßM¿Ç?œ7®˜¿à}€(¯K³¿ìÁ=ÐE'¿ïÿßHÐSjUNASNone?†úVv²±?ƒÑ7ù0'?臘'Ý5?ƒÑ7ù0'?Ì8aÒ]b?—_ÎåhH?ïˆÏx¶‹?—_ÎåhH?›±7p»'?;E©!?ï"wDz'?;E©#?•KPŬ?€°ºOm?ïWÕ§eyÓ?€°ºOm4FGL J1712.9-4105?ê8Oäˆ$¿ò—7¿‰î+À:NM6êwØÀ;qäõ8@#Áåh$,?ý"B
y?Æȶè‰ì¨¿+L€ûµ?½YVˆwÞ3@cho«­?Ô´­Vœ¿ïùͶט?ïùÞHS'?³LyKµ¿ï€Ê`"?ê"ÄÀŽÐéUNASNone?ï×µuø?t0€÷ÛQ?t%EuxÓ?t0€÷ÛO?ïÄøµD?¬»°Œ9D?}ƒüý¥^©?¬»°Œ9D?íUû·¿ÈÔ?¢B|)ÍHÁ?µP"B¹_?¢B|)ÍHÁ?ïƒ$Ã×,[?'7…½×X?6Ï
4éD?'7…½×Y4FGL J1713.0-0521¿ìB@'ÐZ@3	Ò9XÀ9±ZI!²À;Š$_ZÙj@_µ֟	@/«|,Ò?ˋ"ˆk?Ҝ"$'\@ob@ÛBà™Þ¿ßÞßHûG¿å¾»öº²¿ëò¢IkƒÝ¿åÈ7½±¿ïóˆ'	?íðh]a…UNASNone?ï:Ï)zð?¤Gåáá{ì?˜®Т?¤Gåáá{í?ìîf. ó?Ç2ƒÝԋñ?¸ŒÏVŽøi?Ç2ƒÝԋñ?ë?×q%|Ï?­Pg`¥ý?â;jÅ?­Pg`¥ü?îÐpãÔ¿Ã?"¯É0|á²?¢øñ´ß?"¯É0|á²4FGL J1713.0-4236c?êxßÚXšÀˆãƒÈvýÀ9t«ášº+À:Î	ԕ+@ Q(;³_@såÍNÓ?ÏÔ߀Xªç?Ïo¹vXÌË@ía¥6…Î?ýZ
…#ÀÏ?ï:`Nq¿ávŸLa¿ÜI@¢B¶¿ãy[k`¡+¿éÊìW¬@¿ïóGŠÙvUNASNone ?؉;à@PÑ?Éû"•àöz?ã»bßט?Éû"•àöz?ãˆj´+j‡?Ô	Q¼\Ù?Øï*—©*ð?Ô	Q¼\Ù?Ýåçmßu/?·†Pÿ«5Ê?á
IEh?·†Pÿ«5É?ėˆú0Ìw?­Í[6›Õ?êÚÁsÌâ?­Í[6›Õ4FGL J1714.6+3228?à[ídºã@@ÆÂT£ÆÀ;ª{jÚinÀ<äŽ^Òô.@!õè?û³5L'?Ñõ£KÛ¡?²º·¡lvÌ?ã'3¡m"˜@O?w9Gt¿ï îzÔ]?ïò®Þ¥<e¿Õ'*g2¿ïá.žxük?ï–kFŸ÷'¿Ü¾ïÿ×¼UNASNone?ï÷'B<²? .«È­¥¬?PÛ{Նœ? .«È­¥¬?ïþ	Cî–?Kg"Ý
?.kÁ¤ ?Kg"Ý
?ïÁȞÌÈ?ˆ{ôàÌ?ˆØLÎ#?ˆ{ôàÉ?ïþÙ>4ï?$X-òH?"ḻ 
?$X-òr4FGL J1714.8-1421¿ã_û>ø̏@+·+ˆDÀÀ:™âàíÀ<Fƒ
â@Rzé*?úË$£Mx?׈†KÞû£?áÂZ£Š´@E܃#6@AmÙ!næ¿ï""Ÿ´»´?ïýuÁÎ#¿ÚñÞ"Š™¿ÕÝÏßäØ¿ås‡ìÈ뗿ïý
a½_GUNASNone?îš	Ý#%?§M•7N$?¦_b-Í®B?§M•7N$?îkž:°?ºªýÁÏú?©FW/Ôú?ºªýÁÏú?ëCÏg¨?¬ÆÖ4¶A?Âðþc¥\?¬ÆÖ4¶C?ê
ÿ¹E&?¬ À3A½?ǗÈëg?¬ À3A½4FGL J1714.8-3849¿ì"üۉƒn¿ÀéÕÖX½À8@NÕP)
À9Ì:䜸@—áŸ@2êRï'?Áùh6J>è?͉—Bý*¹@Û%ö3Îd?úX»¾¶S?ï¯Ö燿åÌÞý';¿àKeè'%¿åìŒñª²¿ìV/n¿ìêßBEJUNASNone?'A£•§§?±š‰½ý
+?ïmòãRÂÇ?±š‰½ý
+?™
=î"Ì)?«ß
¡åÇ?ï7–‹a ?«ß
¡åÇ?­£"•¤?¡¸Ê7ÿ;ÿ?î%Ç綮–?¡¸Ê7ÿ;þ?hÎ_`ð	?Z`Þ¹6{?ïç1 Ÿö?Z`Þ¹6|4FGL J1714.9-3324?ævqÓI@ö¥
k#À9oNäHÀ;*¯ÿ6¬d@ÅÛêÌçû@òzÞÃo?Țk%½Ô·?Û}¶Äͤä@5" ¼8?óH}ˆkI?ÚZÀÀÏéb¿ßð½Âôu¿ÜZе
¿ä3ò«ƒ¦é¿ìl¸?wT¿ïþ'¼ÞB@UNASNone3FGL J1714.6-3327?nÈ^+ê£}?uTk‡ü=?ïá7¡Ô\?uTk‡ü=?› L{q
5?¶k¢£L‰?ï"ýœ$w–?¶k¢£LŠ?œ'û
q&?Œ'œä&Å?ïè'¬wN?Œ'œä&Á?zûª•'†?c'Y€Ú?ïËÒªÔû?c'Y€Ú4FGL J1715.7-4239?î_ð
r?ÀðCRe(À9ì) ã9÷À;­e(xÅ@¸dC¡j@õÆÛò¾?ЂV¼¥7]?°	ž¡l2?èk¤Éx"v@ٍ\õNv¿Ûàÿß"?ï¸x·¡Â]¿è3¤Ýšzj¿ëU—Ià?yë‰%ƒU¿ïÍõ´L£UNASNone?îð½ér:'?£/£èμ7? ô!hÜ]š?£/£èμ7?ï¸-ÐhÇn?«aƒò™µ¹?ô‹åÎ$ ?«aƒò™µ¹?ë,ägC
ó?°Å
·Jž?ÃLnbóÈ5?°Å
·Jž?ï}Ÿƒa\ò?…A9¤¨g?L"Ôaë?…A9¤¨g4FGL J1716.1+2309?ÞÊ8/–":@>§T~–À:}ÜygËÀ<~¾b¦¾@ 4‹Âktî?ü‹vUDz²?Ä1}{€Õ?ÂFÒâ»vŽ@F}ÄY?ú<–÷RÝH¿ïiaB?ïÿîbHÊt¿àVà¡ë͙¿Ég]äâî¿é
Ä^ê<¿Çâðµ	UNASNone?梁L»µe?‡ÛÀjµ?†'lѦm?‡ÛÀjµ?îo?ÿò™?¹ó$_mb?§	ւ?¹ó$_mb?î؉×.»¦?˜ƒ@²?¢wbE¥?˜ƒ@²Ÿ?ê"x²Égà?°`Ïêý?Å®4Ú`?°`Ïêý4FGL J1716.1-4342c?Ù<£š"$ÿÀ	U°5½Q/À9§>ïÿ×¼À:îfWLíï@~Êö†@¿–áXu?ÒéWG²J?ٗ֠áž@
/Â=&Ñü@-ø¦š^?ï
užèó¿æ"_@Ø7¿ä˜=Î펿ëÉZQ…-Ò¿äس|
¿ïÿäÅøUNASNone)?ܛŒ'mÖ?ÎL)^'LI?á²9ÿ¶É?ÎL)^'LI?áåvÕx$ø?Ô^š9;-k?Ü5U¶?Ô^š9;-j?Øü³G7ì?¼Ékí_Ìi?ãó¦\d
?¼Ékí_Ìi?Ñ$vÜÞ÷?¶R䝘;L?çmđô…?¶R䝘;L4FGL J1716.9-4152?íAJ¶ÀÖÆÞvB|À9½laR*oÀ;"÷í@'qÓW@7"¹hkú?ÍWÙu&É?ʧ"Är¶+@j <¶i´?û†2(œ+?ï5¹pޏ?ïg,_›–¿ØÝZ»g¿äE‹àsr¾¿èªÜb§¿ïþîB=g?UNASNone?àï'?üş?ÏÀ9ÀØ7?Þ!±€tÃ?ÏÀ9ÀØ7?㙾q/?ԏ͘÷Ê?ØÍðƒ÷¢?ԏ͘÷Ê?âôbQ#?¸XäôÀ?Ú;]¹õÉ?¸XäôÀ?Ñ29dí?·d7à?çtæûãMŠ?·d7à4FGL J1717.0-3218¿×Z‰»–¦ø@
WýO0ÀÀ9älòq¢À;6q'Šˆ…@ íãLì@¡ÞËÒÒ?Ã*[sCD¿C10ǾZ?¡ñ,}ŒrÀ@Õ®zÒ.6¿ã'㍲b?ïœ)@ìt¿å,"½ð¿èó`_fAþ¿èkÆ¢'9ú?¸ˆ_	¥Æ#UNASNone?î9™Dɝï?°¬Ù¼ßº?¬fk³f!?°¬Ù¼ßº?ïÄuÿº?¤ÿp¹U?}öÅ"ñ‰?¤ÿp¹U?ìzºå»gX?±‡l?7Ë?¼*(Ò$Å:?±‡l?7Ë?ï•~"êá?÷ ÀÒ?Š¸`[Gà?÷ ÀÑ4FGL J1717.5-5804?ígšlìzÀ'hRÀ:kàèãƒÈÀ<~Êx_@G2?˜F]?üX#ã4_?ÊÚ*BôœJ?èð¾C
Â@5I¢
c@¥®¥ÅL?ìMIÊNmK¿â¡Ý_ìû¿•ˆÞWÜ¿à8IÝï‰æ¿ïÆd""T‹¿ïý	«zl®UNASNone3FGL J1717.6-5802?œÖG§¯†á?±†mù,±?ïMƒÉ?±†mù,±? [ßÏÔ#?­¹†bòØ?îúB½?­¹†bòØ?²¸L¿ÏF?£P•Ú¬É?í¨öh?£P•Ú¬Ç?£"pî_g?'Õ@æ?îÆÈñ
?'Õ@æ4FGL J1717.5-4022¿ÁnÈ— ¿÷SŒdý±À:–Í[h£À<Br©jÈ@ B–áÙNe?ÿƒ\=¹?Õ2køvžÃ?ïùƒ^ıu@á¹Þ³?ý:˜‡ É¿ärâ?û˜'¿ïÿä†ýµ£?ïþú·Šñ¿Ø‹*k
•¿ì°¡óÛ/¿ïé˜_‡ÏîUNASNone?Ç'•k6ˆ9?ÇI‡çO›?ê6¥2]ò?ÇI‡çO›?ÆÊp˜¦U?Ñ_ó'4'Ë?êMcÛÙÖj?Ñ_ó'4'Ë?Ó%¥L'ó#?¶¸o{GÌa?æm-Y·o?¶¸o{GÌb?¦ªÚ¤)¯}?¼Ü]øü{?î•RU½e?¼Ü]øü{4FGL J1717.6-4404?ÏÙk@/þrÀ¿¸fä;À9"šv8kÀ:Ûµ#bۗ@f_>ÿÅ@8Z\lèa?ÒI䥆?ÕޏÂÖ(ì@Dy¬"H@n"³*å?ïüPþ .‰¿íQ9®ww0¿ÞJªž#Áü¿è¬Fàˆ¿ë•¢ß='³¿ïúÂÇ;=UNASNone3FGL J1717.6-4404?ç2)yÙ¹Ó?Ë1‡ä­ì?ћ­LŒY?Ë1‡ä­ì?è"ônH©Ÿ?Ð¥¸¼?Í°.FÝY…?Ð¥¸¼?ãÕè2€#?¶ìŽ¾i¡?ÙÆT/šÿº?¶ìŽ¾i¡?áFËC÷\?·œ{l·B>?ÝÿrixH?·œ{l·B>4FGL J1717.8+1955¿å3]³ÙÃ@=1	¾ºÀ:Ë:CȬ­À<bw‰¤Y@Ú Gs1@éºÿDï?¼Ö_Æ?"žgšÕ*?À†D}2…¹@¯Sj5S?CtÉÖ¿°Å'<3¿êþ'âÆ3V¿èdµVŽ'¿«d]D 7пè™ÇâWMšUNASNone?ïz¸ª'œ?‰½Œ4¿/Ô?ˆ¡QÕ_Y<?‰½Œ4¿/Ô?ïýFç-®?T§ô>,^?5ÈƗJ†È?T§ô>,g?îÿ8K®?"§ˆN
? v+E$?"§ˆN?ïèA‹UÌ{?\»ßŒu³?g¾tª3"Õ?\»ßŒuº4FGL J1717.8+3925?ßfïÜÉ^@A†
¢À;Uî:ތÀ<ɓnÝ-m@ ïñ2@º­,**?ӟ¡[¢?Û>.cëŒÖ@û$ p¸Ð@¶ÁȌ̿ïýíÁ?￧¬_o¿Äó¡ã?*¿åB˜Ì@)¿çï…^y2¿ï¾­àMˆUNASNone?ïc#MwÃZ?".ÚCa\R?"›–Q"Â?".ÚCa\R?ïÏ÷'?}LÚZ»?xu"1v7…?}LÚZ»?íO'P&7?£›–[¯ûñ?µ‡»u~ÎM?£›–[¯ûñ?ì¼ÀH¿"Z? Šht\E?ºýº]4? Šht\E4FGL J1718.6-5821?êöÿP
XÀ'ø@À:
ùûAÀ;ǁ]b±¦@Õ0‹yp@}G8£µ|?ÁÙ¿¤p7K?´hÊCÛw
?ðŸ-݈ܳ@•»ô7tá?ïÆTdÜ#¿ãªÛuÜûï¿æî!7¿äNMÃiÍ¿îÐüqÖ1¿ïîDنUNASNone?ïâÔñ€?šU¿Ë?£¾…aÐ
?šU¿Ë?ï­}rƒ¤?©'Øó™%?œ
PQ¯‹~?©'Øó™&?íAÈ#J&P?¥1iרà?µñ¾å®Í}?¥1iרß?íC£öTq?¢ì¾yV?µçjàM\|?¢ì¾yV4FGL J1719.0-4038¿²níîl¿ýeÙ($â8À:|Í°ø[À;JuòËd@ µY€.@aøDIÜ?ÇÚDºõŠ?¦C®Öl³²?å>ÖÕdK?üAòMå¼?ï­o¤Ó‰¿çN>f˜¿å<â¿'r¶¿å]'«ŽŽ¤¿á£Ž_©³Ã¿ß1ßá|‡:UNASNone?ïÄ;‹á?x¥íVz,?}òâtºÎ?x¥íVz*?ïSQ
º?°Ñ¦ÛäMË?••Þ_ž(ž?°Ñ¦ÛäMÌ?îz&'‹?›/&à?¨]ŸÍ‡çJ?›/&à?íKœ—+Ë'? \8}Èy˜?µ£F¡¦Å? \8}Èy˜4FGL J1719.0-4221?ï
äAD¾¿À v}4ßÀ9Á•XÂ8õÀ;A	pÂ
@>nfë@C{Ó?Î!4x®?܉+bYfy@LeáÜ(Š?ök¥¥–}?ïmq½²}–¿x:ì1ŽdÕ¿åYxâií¿è— Ÿ²¸¿ëɉDH"¿ïó<7¾³/UNASNone?µ,W¯¤v?¸ržÖ´?íZu
ëq?¸ržÖ´?Ì&mËSb?ÐáË·ŠçØ?èöd»M+'?ÐáË·ŠçØ?À(˅$?ªÕéspÇ?ëú`5Ͷ?ªÕéspÅ?}Û×ðZžB?f <imŠ½?ïÄHPJÃ?f <imŠ½4FGL J1719.1-5348¿ïvi?fâ{À"¤w¯dÀ:hRGËp¬À<¿¨!Ù@…"|NZ+@–žh5s?¬Gq-À?@‡1Ó?Ñ´âË;Ó@×nŽ¨ú¶¿îJj½
<)?ïò§½HËK¿Ý·DdÞÑÝ¿æ'Ê !Èþ¿Û#¾…â-¿à9"¿ºëyUNASNone?ïÆ=­…yN?zm5Ք'?|á)=CYh?zm5Ք'?ïûë⑾Ç?[Ÿ·4ƒ'v?@Pu¹æ`?[Ÿ·4ƒ'v?ïK+Ž?‹4"p?–š-ÿ®>?‹4"o?ï®\àHññ?u™vÄAF?"hÇíÃÕ?u™vÄAC4FGL J1719.3-3424?ëü¼‡-©2?û!Â]BÀ:d%B{¦À<¦Á Hà@ƒžçŒ@Á@ľ
'*?ՈŽÄÔZá?ïú›ýwª@'
=p£×@Âè/SՕ¿ä‡Úà
í¿Ó§üÞ¸\¨?äz؍Út¿äém
A"¿ïüª£´P?ï@ôQvYUNASNone?ŸMÞ+'h?¦¢_ßќÍ?ï'§~Å?¦¢_ßќÍ?£•Äâ™[?ÏôB‹‰±•?ëWŽÇYª?ÏôB‹‰±•?ÅÂy°Éôy?°G…"€N?êa"Í'á?°G…"€N?µ×²#?¬DÝèe?íE	»œÜŸ?¬DÝèe4FGL J1719.4-2916?›nÿ…Mî@n"$咖À:Q'l~®\À;UÎ{"¶
@!uÇ,yÜ@E¦'¶(F?Öââ7î?Þ¡x ¥§o@ ˆC0y@YKË°m?ïR…sq礿Ý]+4¾y¿ç˜Æ‰ˆ*¿æ¡^X¿îÚÑb2Ð¿ïþ*ÝúºUNASNone?ßÉ]´?ÌèËÕ´Iì?àQ?{¿&?ÌèËÕ´Iì?ØþYZó¶…?ђeb…j?ã€ÓR†$½?ђeb…j?Ý-"B&Š?¹4ó[8¨(?ái8nÞìº?¹4ó[8¨'?՜k1˜Þá?´Öà-zÉ?å1Êg3?´Öà-zÉ4FGL J1720.1-4358?â
ܞFüÀ<Á^ڀêÀ9†¿:¬¤À;$G4q÷"@á›þMÎ?@…ÜMsP?Æ[yMsÑ?ºþv½÷qç?øýÎè/ÿ¢@9öw– ?ë0¿e†?ïx5›Ã?…¿éJº¾­OY¿äËZ;µ¸´¿àqÁŸ:¿ï¾ÿ—$tUNASNone?í1D4È?·í ðsË?¶uß÷~YÅ?·í ðsË?ëÈu0mëœ?ÈÌZ˜!?ÀÞ+>HQ?ÈÌZ˜!?êÑ%¤ò?µzy;Á¶…?Ä»¿ioÀ9?µzy;Á¶…?ç"G²yy?¶âThÜ?ÑÁ»p›
?¶âThÜ4FGL J1720.6+0708¿é‰§ºž0@7kDå^³À9×Ùµ›äÀ<àŽJ°þ@´fêD×Ë@Yܚ )×?Á#Q(f¦}?Ù é¤@ŸË':)Ç?þ¶§NŽ?ïý$ƒmj¿Ñô;[uǂ¿áäÊE¿ç|卍ó¿ìÞÛÃ	Õl¿ïä1‹@UNASNone3FGL J1720.7+0711?{˼>{nø?Öö
¡!?ïÈh‡ƒ	#?Öö
¡!?Œ¡Õ2¥ãF?"xÚût?ïx«5hs?"xÚût?—:ÕJ5˜?Ž¾ÉE¨-5?ïF)U®S;?Ž¾ÉE¨-5?¡ˆþ´Ž?ß?‡FõGþ|?îçp·?‡FõGþ|4FGL J1721.3-5257¿Ýb¾""pÀ"AiÂ;ySÀ:%ÛÞ¸‡›À<$"û¥'l@
5]/@ô·Í?Åï"77y¿?ãªØ¡e@ëÒú
w¸@Ù¡û½Ñ¿Ï2þ'W¿Ý×&¢¬ì¿ÜëÀ š¿é_îbHÊt¿ïôù è­Ô¿ï%m
ÊUNASNone3FGL J1721.4-5253?"u
½sè?·›·
2?ïdW—j`?·›·
2?©¨…$§?¯…Çþ[®¼?îoEw­¾…?¯…Çþ[®¼?¡Ý$äFZÉ?'1ۓkeÇ?îâ-±»šT?'1ۓkeÅ?«{e®áÇ?qÐí£Ç?îHI¥ã?qÐí£Ç4FGL J1721.4+2529¿âó]òmÓ@>?§e47?À:sÿÜĒÀ<DTž½ÅÉ@Œ¶¦Å§@æù[¡†?¤#
q¿¯—%ÿv Ï?å&-'2ÂË@ú 
÷Õº¿ÓÀŽ%D.¿ê–-žž¼¿éÿ7T*$¿çñ"'›¿ãæþÜêQB¿ïæH¿™UNASNone?ïøæ‡.œÑ?PЃ2•†¨?LeãEŒºÅ?PЃ2•†±?ïñ¥µ!¶?EEs–Õ#?\´•½Ì'Ù?EEs–Õ$?ïøQ›Mê?~ˆ/NŠ8¨?~#×2Y
Ñ?~ˆ/NŠ8§?ïã¹~Aù?_ûèê}(ª?lFí¾?_ûèê}(®4FGL J1721.4+1131¿×ÉUS'Ä
@9$ƒÛÂ3À:Eóå?ŠZÀ;íåf ÆI@dˆSöø@('»0Ã?Ä\|,Ì<?µÛ.dlf?ñúÑ!Æ#e@Ley+ü¿ïä:Âs­w?ï´êB~¸¿â7¨ã¹x\¿é¡nD9Q¿Ü4Â_5š—¿ãƒö.Åæ)UNASNone?áÓL?ŽÆŽŒËBn?šÇ‹>í%?ŽÆŽŒËBn?ïï×óÉY?{)¿Óé0?`ú(6¦Ö?{)¿Óé0?íÛ·>Âàø?¢
DcîGÃ?±"F	èøD?¢
DcîGÂ?ït ;T?ŒY»´Þ?±}ûø•e?ŒY»´Þ'4FGL J1721.7-3917¿ïÛ}ãý'<¿÷ÝÚ;JXêÀ9Pè0-À:ÝîgQGñ@•8"Djé@7褙§Ü?ãRÿ" ?Ð÷Šûñþ`@À ìߒ?ûË …¸Ò?çi·ßTä´¿Úzµ]šdñ¿å^ê–p¿àuT«Rÿ¿ð?ïþ¥¢fqÏUNASNone3FGL J1721.8-3919?Æ.o׈[?ÓF®ËTâ?êtd8Êé?ÓF®ËTâ?×ÿ:¸8c?ԒÄ ./?äb£øãÏ?ԒÄ ./?È|¾lwÛ¼?±ƒüæL–û?éàÐdâ	?±ƒüæL–û?¿Û…è؋¬?¬kE¾SÆ?ìBäî‹?¬kE¾SÆ4FGL J1722.1-4007¿çÌMs«2À*¼¤¡5À9q¼´i)À:þX"»@=ó~'W0@µiF·G?Êl‡"?Ŝ¢x†0@Bõ:ªú@ͳ\cX??âøC]¢Èl¿ÜQ0^ƒ¿ä¸Çâ'@¸¿âs,þåÑ¿ïOÙ\'H?ÔVˀœUNASNone
?ßf嵿¨á?Ëð[§zm?àL% +?Ëð[§zm?ë·`.Êé?ɧ–9[?Á"D×äZ?ɧ–9[?äYžMêI?¸ü0Zž.?×LÃd+Ío?¸ü0Zž.?è¿Ü'ôí-?±Ö3_¤ò?͏`,KL?±Ö3_¤ò4FGL J1722.1-3205¿í'+å™À@Mt­P0À8Ù¤K¤CAÀ:³*dW˜m@ñ+:ÁG@ø¼²£V?Õ²½?É[¼>_@a~4¹E1?û/-4k—~¿ïr> wæ?ïýéÚúŒù¿èÄ¢'ßܿ䅠ž²´¿è)ó¹  ¿ïÿ´ìw8UNASNone?Éȱ‹¸þ?Æî|¨z'â?éÓ¿]Á?Æî|¨z'â?®ŸJŽ¼E&?¼Ÿ¶Ï>½Ë?îW;®?¼Ÿ¶Ï>½Ë?ؼ}Ô…?¶òðn¡d.?ãø¡Áú=?¶òðn¡d.?Á¢½ý‡‡?±ƒ‹QÁ?ë—P€¼Þ?±ƒ‹QÁ4FGL J1722.6-3135¿ïå¦ã‹ô@¹^ƒCÿÀ:m^º z^À;üVÈc±€@XýËrYº@Ú³R¨D?փže[N…?îù¶9ãP@Z5Ö{¢?ÿ‹Þuk¼ç?ًÛk¡¿è×n~ÓE¿Æ~h»«<Y¿Ü	ÆTㇿïÿý{ÁA~?h$¬ˆUNASNone?Á˜ˆD'=?Æ4I›,?ë™ûîö0?Æ4I›,?ÆÐrú×š?Ñ[ÖÒZ–,?êKãAJ<Ú?Ñ[ÖÒZ–,?Ќ8.b¯?¶çǀm?ç¹ãèñΩ?¶çǀm?­ëßÿ%)z?¢þoU
\…?î!B
­h?¢þoU
\…4FGL J1722.8-0418?í¹b"‹hÃ@1z¿¹¾ÓÀ9£ÎµÛÀÀ;ƒ¤Ùš;@Žy&²qW@òÜ`¾†¹?¿È`g¯ù?ȑXJz@é{f¨«…@d]!Ä ¿ïúþ8£N?ïþ|¿á
Æ,Ÿ›¿ç?!þØb­¿ä…ºŸM¸›¿ïÿõMõVYUNASNone3FGL J1722.7-0415?åÎùհݲ?È?¥ue1œ?ÔbTžD™?È?¥ue1œ?ÔüŸ£¥Ï‹?ӏTàeh?偰.-:?ӏTàeh?â¨HU" ì?¶:=cÂq"?Ú¯oT÷¾)?¶:=cÂq"?ÒýlŸ.¶-?¹ÌQ€~ ž?æI°h¤é?¹ÌQ€~ ž4FGL J1723.1-2859?å4•8g@_\ÔmÀ9áºu²3ÄÀ;U';&F¼@¤š"i©½@ùB%?Ò*5}æ4Ó?ß<eáÜ)@ÅSü×V"@ña£Êu?Öû{8…ƒ?ïäÕ!…
ì¿ç²™0¬¿è:P(6ï¿ë»¹.׿ï®
4»ÉUNASNone?­Œ¿ßë¸Ç?°y9;\{?î'4Dt?°y9;\{?´X)R^À?À!ýÒ°?ítúÕ´'ï?À!ýÒ±?È9©|\?²³Å(Ì^p?éþñŸ• è?²³Å(Ì^p?»{ë'?ÏR?¤žÙHm9?쐂Ø?¤žÙHm94FGL J1723.5-0501e?ⱟk觵@0ös>»ýrÀ8¥½áw~½À;Gýœ@ sÍ$™g?ÿæI ]?­'—¾V迅'LmcR,?ÝÉn"æW@BØ(J¡å?Փë$%Ï¿ãÎý'¬¿ã©yámm¿Û1¢åGÂâ¿âCuÀÌcp¿ÆÑM$ ô,UNASNone3FGL J1725.0-0513?ï-Os;K¶?•‡!¡rÖ%?šV˜–‰7?•‡!¡rÖ$?︎)xo?ŸÐ_]sèÿ?Üu¡ä<î?ŸÐ_]sèÿ?íFïõŽ{É?§4Né©?µÈ€SŒ!¾?§4Néª?î/JnÏ!?—°1´yRV?­;Y
ð?—°1´yRU4FGL J1723.6-4126?¸¢ ËÀž'6§À9È.5p¿À;/51:4¯@'')Â@8M[Óem?Îàw	KÙ?¿ƒ"´µÕ?÷ÞêÁªYÛ?ã×vŒ#d^?íu–Ob=ã?čsñidH¿æIÅ$½ú¿æ—:yx'â¿æ™Umß¿ÌD87SÿUNASNone?ín"uV¡?½ÞóÞÄ?·Ô‹dUJö?½ÞóÞÄ?çøwmÕËÞ?Óþí1@¤a?Ð$ThB?Óþí1@¤a?é;…²:QÌ?´í4Åu?Ëé7¸Ñ?´í4Åu?´kãÙÔ¤?œèyÈ:Ïl?írƒžäÅl?œèyÈ:Ïl4FGL J1724.5-3008¿°RÃâiª"@	aâs'?À:©¹¢MÀ;£­X"?
@Oe/Û@Á=¼#1?Ónä#Ösë?íÄÿxñƒe@zbœ­J?úbԘôF?ï^ mÿ¿Øꁺè¿áæ">iƒ¿ìªx^¶n¼¿ïÿÿ" 5•?á3Ê!Ì®oUNASNone	?­'JãL?´Ú»é?î-ŽÏÛQË?´Ú»é?ÀåBòçõº?Ϋs)›I?ëƯCF'?Ϋs)›I?½
Bøî-?¨ì4Ԕ­?ì^­÷ â:?¨ì4Ԕ­?†ZÞ)š?oçê	?œÀ?ïÀóJC­é?oçê	?œ¿4FGL J1724.7-3737?¨ÖÈð¿ð¿Ï"èbUÀ9L‡?$>À:Îr«G@O²{<â4@YH;4Ž?ÎqUää?Þú™#R @
.9™~Á§@rx¨ˆIæ¿ïâ7,¼÷m?=î"2¿çù҉¥/пèsGà¿Gÿ¿ç!ßMØÑ¿ïÿè2_NUNASNone
?ÐÒYŏùÉ?ÊúïTî_!?ç–Ó8?ÊúïTî_!?ÆìÒ~0Ã?Ì#¦<ÁíÖ?êDË sÐ?Ì#¦<ÁíØ?ђø"Ç
?¸wç20£0?ç6òµœ{?¸wç20£/?Á=ðPzÆ?­	Ÿâ+c?ë»°ƒëáN?­	Ÿâ+c4FGL J1725.1-1924?èwj«b&@"ˆP›ùÆÀ9Oç"!°TÀ;‹M@$³>@FíùXŒ@_ž£Ä•Ç?½uQçÿƒ?Ê⬩@3ٛè(s@@~æ?ïýüºÑ!Æ¿á'Ñß^¿â7Š`@²x¿äè‰÷e&Ë¿î鱿«&4?ÚD¾@BoUNASNone?Ö¹Ù›so?ʛQ«b?ä£v²FJ?ʛQ«b?ÒF)äøl°?ÑÎo¹¯ ?æÜë
ƒÉ§?ÑÎo¹¯ ?Úp9
³›–?¹Ê_JI?âÇãy&25?¹Ê_JI?ØvÎC"°?·Ó6r?ãĘÞ5û¨?·Ó6r4FGL J1725.5+0840?í\}Vwœß@7t>–=ÅÀ:8"ïïÄÀ;ø³ÓÃt@o‡]s@®^L¼q?Âv'ƒzÉJ?·4—¡Ç»k?ðÃmrÊ!ø?ûF°¨ÿ¾¿æáÀå7ý¿ß©jÝn…š¿ë¢†ÝÕ2Í¿àÀœ2#i¿ïýR¦–_¿ÝŠºC2YÄUNASNone?ï_V@ýL'?–êdΩx?"7àVoÍ?–êdΩx?íθÍÖ
 ?¾>bA¼Ý?±Š9'O«?¾>bA¼Ý?íšVÏß`‹?£˜'èë?³-Iû¢?£˜'èë?ìò)6¤?¨äñ]â=?¿oö¶Jé?¨äñ]â=4FGL J1726.2-2903?ë«ô¬¿Ô@'cj2¤À:3±6nQÀ;x'æÏ­R@Œz@ÎÀ§¨?ÒD@ ×f?ܺé"Ä@	Yšäó4@e
˜ÄÝj?ﶋ!±«‰¿äÑï¡c¿ÁáBWC¿äµüŸ|2¿ïýX «Ó¿ì òʍWUNASNone?Ý<ðv"o?ËäS5Cé5?ása‡ÄîÊ?ËäS5Cé5?Ôt[ˆXU'?ÒhË4²êã?åÅÒ;ÓÕ7?ÒhË4²êã?Ö 9µI-ð?·äNËvr\?ä¯ã%[i?·äNËvr\?Ñ>släj¢?±£
ú…?ç`ÆIÊ®?±£
ú…4FGL J1726.7-3930¿î·ÏåÝ	bÀVq¬ÆaÀ9ÔÙb…UÀ;>"à4ê@>=I·™@¶
~C›?ÑkøvžÂÎ?×(Õ_°@Œq'êS@ØéÆW½¬¿îo<c]j?ïÓpöa7¿åƞµbLü¿èÕ·UlC¿æ¶9­ ·›¿éàbiªUNASNone?è!+B+\?ÇAtŸZ€Ï?Ï{R÷ÃR?ÇAtŸZ€Ï?é؇«#ÈË?ÐwÁîoø?ȝáSpÜÕ?ÐwÁîoø?ᱤ ™*û?»"â,ASD?ܜ¶¾Íª
?»"â,ASE?äÆù´gùo?¼üü©%i?Ör—0
!?¼üü©%i4FGL J1726.8-2659?ÓjçÛÏ%¸@$ý£.mÒÀ9º`@²w·À;_œÈù@Bm¬@<eü´%?È÷ùñÉ?¶éÀ£s¸	?ós̀v²å@ýb–Î
?ïÿr ®Ì1¿Ý§š
\à¿ë'ÑÀ§zƒ¿Ùµ'm¿è1B}Sö¿ïÿÿ&¦³UNASNone?ïbµòø?£{íZÙh°?"©N_Á ú?£{íZÙh°?îK‰âb?¼+ś¨Ò#?«GoÁÙÞH?¼+ś¨Ò#?ìI°+X­b?«³Pxm?½²~¥:"ì?«³Pxm?î>ä@ø"?'ÐÓ5'rý?¬»þ0v°?'ÐÓ5'rý4FGL J1727.4+0326?ÝGn=@4:GýœÀ:5N`¶#=À<§Š$Ô@˜ŸBÐà@ —ºœH¡?ÄOI¿;¿Ÿ?њIâøc@V1µ"±«?ùÝ£í¥¬¿ïÿÿ>¹ú?ïÿúŒ—Ó¿ÕÜýë©¿è€#¦Î6¿ã(Hr_™¿ïöÈHٍ¥UNASNone?è‹cTÒH?ÅLK|j2¬?ÍÒr­ø¶ß?ÅLK|j2¬?ØüOW¾'´?Ór,õtt:?ãØT ì&?Ór,õtt:?ä7;ŽÚ"?·Š¶?ΓÈ?בˆãÜK»?·Š¶?ΓÈ?Ójãa‰?µ÷Òi‹ž8?æ~JŽqÏ;?µ÷Òi‹ž84FGL J1727.6-2304¿î3=à<'@37ÿJÎZÀ9O¹ã»ü›À;O¹ïzv¿@åªi @hLŸëÃ2?¿šâÑF?Â½é:ø@€¬:†
Ì?ÿ¥ì©&¥?ïò'íÓ­'¿ç5÷¼d ¿âµ{A¿½ñ¿ä} ½ê¿ãG ñO´¿ïü&Å¢·UNASNone2FGL J1727.8-2308?ì"CÀÊ?·\6»6Q°?»eáù¯Ïq?·\6»6Q°?ሳ£6-?Òà­¦lú~?Ü"¥Þ?Òà­¦lú~?êþ¶~œ?°q—,6•©?Ä&›…?°q—,6•ª?à`FÖ+¢^?µÅ¥§¬â?ß?rS¨»D?µÅ¥§¬á4FGL J1727.6-0849¿é›Ð·òpO@,LÃ\á'fÀ:=LÖrgüÀ;€S`'@ø%ËÁ‰ù@£Ho›?ã/`•Áô?âræ§if@
D7'MLº?ýÔ(ì]`Ù?î'—L¸?¿Óx™q¤ˆ¿åëi~J‰¿çžb¿ïûh÷:^¡¿íòá~µ'žUNASNone3FGL J1729.9-0859?Åm$¾&~1?ȎšzFáˆ?ꤶÐv`t?ȎšzFáˆ?σXÐþ(-?Ðeª4eÃ|?è)ËÀuõ?Ðeª4eÃ{?ÒBsžH/?³®¥>‰'…?æÞÆ{°Ûé?³®¥>‰'…?©Õ@ƒP¢?˜}Vo¸¼?îb«þÇÊö?˜}Vo¸¼4FGL J1727.7-3621?ﺢ/è9Š¿êƒ©8sÀ8éXjËPÀ:6&æô–?@ 2¡'âE@j r}Ì?ù2«¹VÎC?Ô2k€³š@fî0Ê£'@ÜW·L?ïþÝ@7}›?Í.-ºÎG¡¿è¹]"?•A¿äÀåÙ
Lð¿ïÎ¿ìº?äŒt¸8ÁUNASNone?ÝKjž2CÊ?ÔøºÄ€­E?áZJ°æÞ?ÔøºÄ€­E?Õ*!´_!í?ՋŒ¡Šãž?åjï%Ðo
?ՋŒ¡Šãž?Ô·æðú;?´RGÉû½€?å¤q‡'â?´RGÉû½?´&ŒŠ9q?¸Àé;"ß7?í{.~Ž¸Ñ?¸Àé;"ß74FGL J1727.7-4041¿ê_K<Ÿ À	ë9\B 6À:B–Ù˸ÑÀ;Š¶ÂŸLa@'KåÓª@yX`ê%£?ȈH8}õÏ?§[Õ=߉"?ãè"=ƒH@2Âô†Ð?Óì{¿¿éòH‡XNv¿èÁ'ïV¿å'ˆ˜ÀUÆ¿è"Æ@–ž?º3˜ôUNASNone?ï Vdž×?‰IšJUÝ?‡ê}æØJB?‰IšJUÝ?ï½ý;Ìm? A'>¸Ì‹?€€½1ä°? A'>¸Ì‹?î&J[V`?©kNVÇD?­›_úJš?©kNVÇD?îæH÷T?4!©'Û?¡›pŠ¿?4!©'Ú4FGL J1728.0-3550?îV:Š$P¿âÅuà¬ÓˆÀ8]qHA¸1À9óÍêÙþ@,³ô8Ìz@‰µ/ê©?ǃԠ֤½?Ù°ì1"@ªàéºC?ý­¼ÌN¢¥?ïùÐfqN¿Û™¨G²F9¿ãpöBˆ¿éÌòŒyöf¿ídÚu+ü¿Õ£ãßãÕÓUNASNone?©¦Dlòú?ÀKãëæ^?îež;¹0Ñ?ÀKãëæ^?ÂýjfkHÏ?ÌÔÝî"
?ë@¥fe-Ì?ÌÔÝî"
€?§*ˆV"s%?˜_1:
E¬?îWz–¸Í?˜_1:
E¬?{IÀÒòP?g@Ëááà?ïÉlÒZ?g@Ëááà4FGL J1728.8-5131?ï_ °‰ÓÀ"\ú¬ÙèÀ:•:a%À;ñ3eˆ@'hC¶86@¯n'"šV?Ũ%$&Ñ?ƒEÍê"Ò?ÀÇ?EvW?ÿfwM"]p?ïCE.Þ9Ý¿è¼ýÇ%C¿æì€üê¡Ê¿å)	
Å»a¿à[BEÈa¿Û|M"ȁäUNASNone?ïæƒòë¾?žP«]wI?i|ú
A]?žP«]wI?ïé'·/ßþ?'>'
 )¨?fØHÐ ì?'>'
 )§?ï~àòõ©›?ˆÄ•œŒ‹–?#á¡JÌ­?ˆÄ•œŒ‹™?ï³²µ*?orB¶Ñ6?ƒ;Ó{Òµ€?orB¶Ñ64FGL J1729.0+6103¿àVÐ;µö@@³¥ 8LÀ;H!ÔfBÀ<•>zW@moe©P@³ê-/ãó?ÕÈ˒:*?Њ+<™¹O?÷åþFÂ\1@	0=Wyc™¿êë?{@¿èb¼Õ"p¿ãÊHŽK¿èìóþê×$¿ïÕ»Ÿíq¿ðUNASNone?ïû'.¹sw?H",¾WôÐ?A÷E2$6?H",¾WôÌ?ïürz]´Ä?dbè\'´â?<l-Yßß?dbè\'´á?îÔ¶ôy8
?•yzZ¥ß?¢´¸l0?•yzZ¥ß?ïّá&%¼?c‡SY?s7lí"?c‡SW4FGL J1729.1-3503?Ý‹p§sg¿Õ_/:€.À8Ý6ñLÀ:XoÌW@Š
Zvï@QÛèº?Ç¥ÿX:?Õûò•í=@Ç7ƒ$O@ƒê÷Ûj?çÀ;Yrb?Ô¹¥¨›•¿âŠèü®<¿ÞÛ	í¿Œ¿ïk›Äí{¿ðUNASNone?"ìŸðMƍ?±Zˆlú`?ï¬M€>Èå?±Zˆlú`?¤.6ãÁ?¸º­ÀJoÒ?î¿'Ãï?¸º­ÀJoÓ?¦?e½ýÁø?™N]4MÎ}?îœ	¤ #à?™N]4MÎ~?¤vË¢ýœN?SµÍص·?EÐ&;?SµÍص·4FGL J1729.2-2509?Ô³õ²@^øÀ9â"Óa;"À;3Ï`ûÃ@!/z–õ@uýfȌ?Õ6»©?å)Á¿þ]>@CEÎ@j?û_ò+V?ïÿTsõ›"¿ádpݸ­[¿æ}Kà~/†¿ë™ðlF¿ìV¯°¿ïÿÿ)@k*UNASNone?৉#*µË?Ïà¢]'÷»?Þ°í¹ª"i?Ïà¢]'÷»?łZgeöo?Ë£
¹#›?êŸif&'d?Ë£
¹#œ?ÔþnˆÔÀ‡?µ{¦Qó;?å€È»•Ÿ¼?µ{¦Qó;?••€Z1?ÂVÀrœù?ïSW;ÿõ/?ÂVÀrœù4FGL J1729.4-2831?îŽ0ÄkB@	È*ÜLœ'À9¸ª½®KØÀ;_ÐJ/Ï@-ò»ô¸N@m.#(ú?ϝúé×?âÛÛÈé~@‰Æ×p•?óëà;§R?ïÐ•¯)N¿ÙsÇwù5á¿æ(oÀ';¯¿ì6ĸ+U¿æÑôSúS¿ïäîâKd,UNASNone3FGL J1729.5-2824?·3÷øEÑ?¾›ƒù@,?íž÷F?¾›ƒù@,?¹/'ͬá?Ç:¸E¾ºƒ?ìÚ
¦Jd?Ç:¸E¾ºƒ?ȺBy×ç?¶36SJ)?éÿ'oaŠ?¶36SJ)?zþïìS$Ó?n
7äMSˆ?ïÊ 'Y¶?n
7äMSˆ4FGL J1729.4-2646¿ÊqNnÙ¦ž@¬¨ââ¸ÇÀ:`{l‡è—À;ˆÌ&°n@û8|É)T?öœøä'Ëø?ç§"ïQ0?꡵A•Ì…@Ãà{Ö:?üôRÝÊ?ïÿð懈ö¿ë$¦=¿…ãÑZÞ¿å_ú†C{¿ïÿŸB%‹¿ïh‹9"†UNASNone?äÞ9ÎՄô?Ð%
ÈG?ÖCŒbTö?Ð%
ÈG?Ù¼z«üú?×Oî€M?ã!ª÷?×Oî€M?ØD °?´•È¦Ñö?ã÷øÝï¸)?´•È¦Ñö?ØJ¤Ë)Á{?Á
•.¯ì`?ãÚ­škC?Á
•.¯ì`4FGL J1729.7-4242?ß4Á¯O÷À–Â&€IÀ:71xH:À;£¨z-@&‰/=õ@Q¨òÓ?ÔòI~N9Ÿ?äh¿µ<@‰å\ËO@íõ!È}?íD¹ØÔB?׸ÎG*a¿æœ†é"¬ñ¿é‹@•¿ïKtÝøn;¿îÁ†b…0VUNASNone?ØÌØEráz?Òä^(§ãC?㙓ÝFD?Òä^(§ãB?Ðjiakt?ÑdlÞE%;?çòÊËOJF?ÑdlÞE%;?Òúè&þžú?¸,Žg¯¥?悋쀰ƒ?¸,Žg¯¤?'üuæw?‡@±L»?ïhWÈÍ?‡@±L»4FGL J1729.9-4148¿Ð¯9mÖÀºG²À9t(<æÀ;g
"fy²@àn"0žÙ@՟Ú%{?Àu	l?·uPdˆr?ñ>³nW@Ç'¹ØSi¿ï·б]Û?ïÿ´Jõǘ¿ækÑ	ro‰¿æ'á>sÙ¿ànw¬ßÇ¿íBåøí½UNASNone1FGL J1729.8-4148?ﻊØ&b?Šóâõï:p?Iög|^?Šóâõï:o?ïÔÙ}ªc
?™rw"•V?u"A*Îz ?™rw"•V?íQ
Ú£&ö?­Ù¸	>j?µw'*æÈN?­Ù¸	>j?î'|[À}?˜ò¯ÎßK¬?§ßx:Cø2?˜ò¯ÎßK¬4FGL J1730.1-4343?ï'nà­À[ÞM'ÑÀ:.¼ÆÅKÏÀ;¡=ȸk@ª|ÂqU@S°ÄXŠ?Ñ°™É=v?é(¶!å'ü@^(}ˆÂ@¸¢kOYZ?è–Dzƒ?í`ov°`…¿åú´f¤z¿ïý»aëW|¿ïí¼ '+"?ïƒnI‰¶ÎUNASNone?Õ
n+;‹y?Ðgáá+nl?åzÈêb:D?Ðgáá+nl?Ïäyûź?ÑÎê»<sA?èၿÑ?ÑÎê»<sA?ÌR
"¢<i?°Ã鎌Ê.?èë}^×på?°Ã鎌Ê.? wÞϚ¾?'µÜÁŒ¨8?îø'T?'µÜÁŒ¨84FGL J1730.3-2913?ïzÒ?
¬­@Z¡ô±îÀ:Àk<ŽüˆÀ<Y<Íù@Ã÷h+ã^?ÿ{xFbºà?Ö·Tà¬þ{?ïÿp=½P@¶WuÇ,@‰-Vû9r¿ïa.ƒ¡	Ð?ïì­"šB?¨o‹þüIè¿Ó¼_vÞ¿ïÿÿ>¹ú?ï߯BxJ"UNASNone?éL•¨ah?ȗ f$®¿?ÊÍ©^{ú_?ȗ f$®¿?Ã"*™*SX?ϔƏn‹?ë7uYµk)?ϔƏn‹?ޛõßíT/?»
«°<Ñ?à²	Uè?»
«°<Ñ?ÊÜ=Ÿ¬Åµ?·»@ãTüÖ?éHð˜Β?·»@ãTüÖ4FGL J1730.4-0359?ä-íb°Š@/ý™gD²·À9¡ƒJ¢»À<	²öañ@ûŸZMÔI?þ´zuçãª?À_©]ÜÕ?áp'S­Q@B¸A$~?ô˜0m±v¿ï´qV"q?ïÿÔač¿Ãݨè)b¿æ¶ã¡¥¯¿ì´/GhG¿ïÿûÞ]BüUNASNone3FGL J1730.6-0357?Š€!obò?•/¾›	ð)?ï•ÿzBw©?•/¾›	ð)?y«¢ˆd‡?ƒÙîE+q?į̈ºïÅ7?ƒÙîE+q?¢º+ç0t?—ÔŦ²Ò?îÔ]AŽú?—ÔŦ²Ð?Eäkéâ›í?6?µ&Es?ïú†å‡X?6?µ&Es4FGL J1730.5+6018?×ñ væù@@¡êhìSÀ:ǀõ]åŽÀ<g;.ª7@:ê¡tˆ@øåY‹?Ì<"1/?Ç£&
UÄX?ùÐéÅ@X—)§Ä*?àℏFY¿ÏRôčŽ¿éo6žø~+¿ãWB\	¿î{bâMg'¿ðUNASNone?î·;ÝAiq?§$PŠL–?¤ŒB+éhó?§$PŠL–?ï¨'L9cˆ?˜ªÉǞ¨?…ö,ñ§?˜ªÉǞ¨?í¦VÐä¤?¡£œ`j?²ÍOxÚÛ?¡£œ`j?îZÒE7º´?uóHd?ªRÛ¬"TÅ?uóHd4FGL J1730.8-3806?ÓäÿoÀ'¢&0À:@[9âzÀ;šÒרÈâ@LR_žK/@@þ¥Œìã?Ñcêöƒ|?㎻ßê‹Ð@ÊeI/ôº@AæŽÿf?Äöë¿Ý—Š ­_¿Ô«ÉGNÏ¿ãÀ'¢Ü8¿í"rmÛ¥®¿Ý#ÌbïŽnUNASNone?Œ˜NwÚð?'EÇLSz?ÆÆ "?'EÇLS{?Ë"O¤óP!?Џ)ýŽ5?é7lÃ+ø?Џ)ýŽ4?²$rÖκê? OF0°ÚŽ?í»q¥&(£? OF0°Ú?ÁLü-²š?¢ðÛÌÇ]?ë¬Àô"{Ù?¢ðÛÌÇ]4FGL J1730.8-1123?émËd_z@(EºÓ¦âÀ:´Ÿèh3ÆÀ<†íÅjÙ@!OµX«h?ú‡ºt´›?ÕD[å$x?ÎJ>ýìªc?ñL <K	ê?ÿvà.~m™¿ìhûl‰?ïø ÅÝÅC¿æN'à¿±kØ@Ho…¿ä¸
¾
¿Ùj"‡0áIUNASNone?ïã®Ê?nºL\
‰G?lQâ5øÿÌ?nºL\
‰I?ïÐF¡ ?šE¦ãµBï?wõôܯp-?šE¦ãµBï?îvYy€rò?Ÿˆaî?¨šhgøÐá?Ÿˆaî?ï&áÇ»Œ?‹]ømm?3?›#ǝN'?‹]ømm?34FGL J1731.6-2904?ïÐèâǔ@("[CóuÀ:Î.äðÀ;cä|캩@".çßCr?ÿ´o"͊b?ÇB]Þ¨w?£©Þ
aظ?à¹¡Kê?ûë¹Èä
¿ïø…'‹`?ïÍ/(·Ä¿Ä û¸•Ó¿¸Ôç"ŽuN¿æ)S¶`y½¿Ñ'ó—»HUNASNone?ïì­QDi?dÅ\¬è$?cR®»–pä?dÅ\¬è$?ícÅ8!dï?ÇØôŠËù?´áÖ>ô؋?ÇØôŠËù?î#Ɛ%þ? Î6X,þî?­Ã–ý ¤? Î6X,þî?íC5WzêÆ?©.‡šڑ?µæUD(©Ó?©.‡šڐ4FGL J1731.6+0630¿É×5^HY@4®IäO QÀ:ç¦3ÛϟÀ<oyÌz@§5ÐòKa@)¹à<?×ê6jX‹?ïÿæՌŽï@zy5v'@Pԏä¹þ?ëŒÜ­¡¿Ã;—Æ/Ϧ¿ê
@?‹0J¿ïÿCwN7¿ïäÚ_²m%?ïâiamƒ;UNASNone?íódlžT?·Í`ßõ"?°dß$›
\?·Í`ßõ"?Ó2˜¡YÜD?ÒÝu€	N6?æf³¯Sß?ÒÝu€	N6?åU~Yâî!?µ|«õ	'Ï?ÕUL:#¾?µ|«õ	'Ð?ÓEÒ=ž
‹?¾ïbC²?æ]á0ù:?¾ïbC²4FGL J1732.0-2659?ï÷ØɀH @¨5ÞßÀ9£Y#‡Ä…À:2K@]':ØC#@ì=áò?ÐàƒãÏÈ«?É=+Úy]º@ðAFm@­¸#®?áµ "µ7?ïøŒ8ˆÊ¿à0rÄBº¿å?þÞ÷¿ß'Øa*'P¿ðUNASNone2FGL J1731.9-2703c?ãϜìõŽ?Ìf•²ß‡?Ø`Æ'úã?Ìf•²ß‡?âlúá÷Ru?ÔÖhÈ?Û&
<[?ÔÖhÇ?â'OÜe)¼?¼©Ç
?ÚÝ`G5¬‰?¼©Ç
?âšÎc›'z?½…Ê˚˜O?ÚÊc8ÈÝ?½…Ê˚˜O4FGL J1732.7-2559?á¾4Ô̏&@ÞµÛ¿êÀ9Àg{9\BÀ;?÷ˆb9±@ÿ‡ý@k§áZùK?˗©jÄD?ÔÂfa³Ï%@
˽Tn?ùÔ«JF¿ïÙ˜f"³?ïþáòο¿äjd!舿æð,µÿ+¿ì®a&ák¿ïþŽ`€sXUNASNone?Ívßؾu?ÇS·—i?è¢H	úb?ÇS·—i?½‰\›|È\?Çl¸Z"û?ìNÔlfô?Çl¸Z"û?Ȕº4{¢š?±6WœBÓ?éÚÑráZ?±6WœBÓ?·\ñ²<-?£
œË|-M?íaɸz\?£
œË|-M4FGL J1733.2-2915?暑…vÅf@öÿÁßeÀ9(=5ëtÀ:}äÎv@ƒYdJWg@"šVWû?˱AÖäþ?Î^® º4Å@Xùã†M@èîüwŠP?éµâ¥|%ë¿ãu
¸A%¿æîZY‡¿æ@å£]h¿éßb"Ò¿ìu¦à©ùcUNASNone2FGL J1733.2-2913c?΢v_°}?Å 9é'Oæ?èWbhà¿?Å 9é'Oæ?×2#Z­—Ø?ÒèÌ^{?äfîR©4?ÒèÌ^{?ՌCáY5?´™vš•?å9ÞSe?´™vš•?Ó©ºZ?¸g¥#3£?æ+xò¢ôÓ?¸g¥#3£4FGL J1733.4+2235¿Ù–^E&@:²ÙßÚƋÀ;k¬ºÞ¿À=G€ß֕@d@ÚÖb@ÚÂXÖ?Ӂ:þϾ?ïÿ4~ô€@Ù>½ªðÚ?ýCw£ûrR¿ãHƒýP"?ÄYbFò?ïùíÎ à¿çdU/¿ïÿۂr5¨?ïüQ¿æ4}UNASNone?Ã¥H)`†?Êk…¿úÍ©?ë­õ§Þ?Êk…¿úͪ?ÉwçˆwB?ф$®ËÿÑ?é¢8â/?ф$®ËÿÑ?ÊùhwØa}?»Pc6²r?éA¥â	ç ?»Pc6²r?´æê–l?©K'›O?í}"­?2?©K'›Oœ4FGL J1733.5-2950?î|mËöß9?û»gšCÅÀ9–,­®À:í¡(TH@!;rò»Ê@âIC?ð±?ÊôþÑpË?¹6xð+Í?ô»k±)X@]¬Ùge¿ð?ïþ$É
$¬?ïö)óð¿äJN듿çÜÖÐ[͆¿Ã-ˆú:UUNASNone?îf¨öDb?¬Î¥¡ïÝ?©žUp›¹Û?¬Î¥¡ïÝ?ìÉñ3C¦Û?ËjË=ùå?¹°veâÉ'?ËjË=ùå?éÃô£0ü?·ÖsŽþR3?Èð-s?¤?·ÖsŽþR3?ëñE°@˜Ó?³Fz*·?À:é>ýœ·?³Fz*·4FGL J1733.6-2431¿æô=}Þ@hŽ^Òô.À9Õ]z.šGÀ;s‰½×g@0™@
ûÖ¥"£?Ëæá õ?á…X'@-+Ç.'?ýÑ}3'–¿ël{ž†é>?ïùÒSõJš¿ÛÆ~1ß ¿ç"ebZh+¿ì&îRz÷¿ïðx£ÌiUNASNone?€B|ùäot?'òÖÈW-©?ï¾önB?'òÖÈW-©?›ôÔå"'ß?«²
E	6l?ï YXÖëq?«²
E	6n?§Ê¡Ü'ë?">lëÖ#?îƒUâ6áP?">lëÖ!?«RQÿŽÈ*?'g¬«Ü?îJÚà}?'g¬«Ü4FGL J1733.9-2220¿ÞeGÉܕ@℁Ú`3À9Ÿ¬îàóËÀ;#J\D¤u@TÞ»·¦ @óà{Ö:?Ñ,à]Î<d?à€å7ýO@úuÚw°;?úÞÿI¡´›?ïÅÝÖ´¿ÜGm\¤Æž¿ê³Ãp=U¿íHzøÄ¢\¿ïÿþˆ0»Š?ïõÁ%y·UNASNone?Ý͘ëC†Á?ÑBi"Ðt»?á3Š^< ?ÑBi"Ðt»?ÄÍÜo?͍¸€d×R?ê̈úù¿¤?͍¸€d×R?ÖåÝ/ï×?¶ÿ†½0ÆÎ?ähˆ?¶ÿ†½0ÆÏ?–Õh¢+…?Š²ÎŒËŽ?ïITºî§Ì?Š²ÎŒËŽ4FGL J1734.0-2933?ïÿïIé?üø[ÆÐ3ŠÀ:Jøš°ðÎÀ;ÿGóÐG@ ;<hfç@2Ú˓?ÖöÕ^ìŸ{?ï?CwN7@
º ¢¢V×?ýþ0Çóõ¿ïÿø="ßE?ïÿîÝÃÀ	¿Ú~ߟã5¿Ö¯£#Ûý¿ëtcˎ߿ï´ì`»×‡UNASNone?À=¼Ñ
Ö?Ægݽ¶!J?ëðË¾}K?Ægݽ¶!J?šk³@VQY?²:6A?ï,¢eýMu?²:6A?Օ¸5^
î?µÝ;/K
ó?å5#åPù
?µÝ;/K
ò?"j̀ó,Ñ?…ô'=%™?ïd©"øfš?…ô'=%™4FGL J1734.5-2818?ÜnSƒNQ‰@[»èxûÀ9yÂ=ägÀ:ô˜"¶Ü@F3#îǞ@N¶Ú@¨?ÊöíÈ
˜?纽֏Ä@ð«†+(@úfÛ×+Ë?ïl-_ߎ›¿†ÏÊ¸Ëc¿Û«n®3"'¿í*__6p¿ÚŠ|›1[¿ïûr»UNASNone?‰*«Pí: ?—kIKÕ5/?ï›UR¼K?—kIKÕ5/?¸õqV…G?Ɩ´ZÓ\ß?ìýAQÕ/W?Ɩ´ZÓ\ß?ǂ	p
8?¶z†ªÙ!?ë}£ýr?¶z†ªÙ!?» W~Á?­žÿ.‹É?ì‹íõ'ß?­žÿ.‹É4FGL J1734.6-3548?ÞDQà¿úýª…z'äÀ9Žœ÷+°À:זߪõâ@ /§zùª@bŸYÌúð?à•
ÞÖ9³?£N
ÿòê?ÙOGß=@ú±Â¸L?ï¼Ü)a"Z¿ìe€Y¿ä¡¿½ð÷¿ç8° œB@¿î½©CZÉ?à'F¿,%MUNASNone?îÐk@ã?µo:´x™M?®rùOûñÎ?µo:´x™M?ï@ÉJD?¬Ìɔ{?Œ¹oÍ­nã?¬Ìɔ{?ê—m7'è?­±"Õ'îL?Å¢K#ç`^?­±"Õ'îK?îÔ§Àu¼?•)lhÈ?¢¾Uƒø¤'?•)lhÈ4FGL J1734.6-2912?îŠ?þ2°ì©À9¯mO"¼À:À'\f2@!Jgö…`@`RP/?ÎË]k"?ª]TïÆw?åóø :G¥?ü‹Å~
¿ïW?íUÙP?î>3Æà¿ãí^½¥'v¿á*Vµï:¶¿àç'Áåèþ¿íõ¿4]ÖUNASNone?ìS'ŠŠž´?¿',V÷*?½ck««
^?¿',V÷)?çç-"J¬?Ôx×õ¬'?Ð1¤ÙkÚ¦?Ôx×õ¬'?éB¦Ò5I`?¸»LR~ ?Êõd·*ڃ?¸»LR~¡?é÷fêáÒw?·YÍ/té?È"dTx¶"?·YÍ/té4FGL J1735.2-1640¿ïDF@ ú_"ÊÕ|À:*M)~~‹À;ÏžÙt{@4¶Ë®"¨@ÔbÞ©ª?Äü"_öŠ¶?À'KÊ-á?ùôàM/^@½Ï®Ôi?°4íóc?ï-*ÛuÝ¿ãj'ñ¶'!¿äM'àAô—¿íh!Äuæ?ЧÍęw‹UNASNone?çyóež?Ç]5m¦œ?Ñ
Ú4Ãò?Ç]5m¦œ?î(½ÛÆÊ?½,® 2i?­t"O3"i?½,® 2i?ëB_Tï?®úåKï?ÆöÂ¬F?®úåKï?í_Uu¾?¡"eš0\?µTSò
?¡"eš0\4FGL J1735.3-0717?Â'¢kbm@*":귙_À9iݞ¬(À;l`Nq@2pÃa"@	ÿ&ò³?Á0/GÁ4¾?Ð0&£Ø·½@»)'<†@¼ƒ †]R?ïÞM}·:ê¿ßøQ{¿ä¥žŠš"V¿é+î›S­ý¿ãœ/vQ¿ïö¢¾ÜIBUNASNone?ÉÏL(®"?ÂnRix—®?éŒ,õú"x?ÂnRix—®?¿•v´ þ?ÇPëÅ®¢?ì
\ñ){à?ÇPëÅ®£?ÙB`Ýr?H?¹eZæÉì4?ã^ϑFà\?¹eZæÉì4?¾Xw']Už?¥¤uÄ7í?ì4ñUL?¥¤uÄ7í4FGL J1736.1-3422¿è¼wÑøW¿ò¦J'ÛÀ8ϙ O–@À:ùÞØh'@üpí(@ÐÔ¦2.?¾ÝþMxX×?ߙrb+Š@:Zà÷&=?ÿ=«‰Ü[?ç¹`>.8ø¿áþÐW›È¿Ð•ŽÝ}ôø¿ââ7ùk'¿îõ"€-¿ïø¾nèìUNASNone?gvìa[±?¡ YÂN?ï艞¤ã?¡ YÂN?ŠÁ5ךh?¢Â¦££/
?û(¡–?¢Â¦££/
?'T‹ªg)?‡­ê{ÔJ?ïm[§'¬Ç?‡­ê{ÔN?`@¢ûŽ£Ì?IÎùÁjå?ïï¿]q\?IÎùÁjå4FGL J1736.3-2929?îY(2gڙ?ö¹ïô8À9'7›wÀ+À:¢êºô]5@ç+¶'"Ø@FºÜà@G?ÎUíQy?׺¾A@
†ðÝMM'@1•@C'¿ïÿíUÙPi?ïÿ¾ÇPŒ
¿äXeAxEa¿æړ)=,¿î{J#9Àì¿ïÿèþ†®/UNASNone?Åg»ñúöš?Áô©lFP?ꦁBX?Áô©lFP?£¦(wú?²›@;²?îŞ¯}x€?²›@;²?Çur´žŒ?¯¾\¼¾Çß?ê"¹cRØ\?¯¾\¼¾ÇÝ?­SöýHÃ?¡ÛD‹_Ü?î*À/t?¡ÛD‹_Ü4FGL J1737.1-2901?æa×ÈÃÁ?ø†jGœvÄÀ9Ž™‹VáÀ:b4¡È<D@«šêÒqQ@!dԕï?Ё^ú·@É?ÓÛÊ@«kÔ@¯d9Ö@
7_½ªÆ?ìó0®ôt²¿èmÝ¿è̞
²¿âZ£"Ôæw¿ï鲀ñ,(¿çKù"k9àUNASNone?ÒàÜç—å?ÏîæY¡ã?揑Œ4
v?ÏîæY¡ã?ÒЖ¾Æ³?Ò)öÄۄ?旴 œ¦B?Ò)öÄۄ?Õø3àÀ-?µîñ©Ÿql?åýfŸé?µîñ©Ÿql?Èp™â‹#©?°BzQ	/?éãه]7?°BzQ	/4FGL J1737.2-2808?¦²D¥ûm?ÿÉåA7Ø´À96"S.{>À:Ž"%¼R@сd®M@ßdš?ÏËø&êþ?ÁB%©Ý´|?øXà66ò@²°ÈŠGí?ç
«NÍÃm?Ú#‰<TD%¿ì¼W3Ã{ë¿â¥¥@–É¿çÞÉ^®64¿ïÿø="ßEUNASNone?ãô"R?ÑMég÷öM?Ø÷ûÂåZ?ÑMég÷öM?Þ½Ç!?Ôµ(·\?à¡wo8?Ôµ(·\?ãø@+× ˜?½ê¢?بQ¾Ó?½ê¢?å&r™¦v?¹÷Û7à'¡?Õ³̳Ó?¹÷Û7à'¡4FGL J1737.2-2421¿ï¨2$@
F:À9Ê/¿á+ÿÀ;|ùOâ–@ |}Šsï@èËùh6J?ÀËCòž¿¢Üü@q¤?æüC͇Þ@®r/QŠ?ïË:%•»¿¿ã¾>ê¡t¿ésòí†+¿çqÿÅG¿èVþ"p?Ôåè&Åf§UNASNone?íìÒXº2?°»xÿ'?°™m;z.r?°»xÿ'?ï	rž]Lè?·ñií£?žÑ¬4Vbó?·ñií¢?íE
ˆ0'?£Ìc–î?µ×¯ó¾{u?£Ìc–í?î§+~'"u?•f~˜g˜?¥HÖȸ?•f~˜g˜4FGL J1737.3-5300?æNQûœVÀ&`'ÏR¹
À:–n6>€nÀ<)RáP@Š¿â@inù²Þå?íÐȯܧ¿‹‡¨3
ñ?É–¾ÈÓ@œÄq^'?ä «†+(¿Ú§a£‰¤¿ä€ƒSld¿ã#ý5Je¿æ"!Í°!›¿ØûsT‹sUNASNone?ï߀†ã?jZyaÆÈå?p?¼Žuõa?jZyaÆÈç?ïý´núbo?LËr¦©?2\ˆ,ì†R?LËr¦›?ï¨u#ïÔ?…hš\ýö?…â 7?…hš\ýöœ?ïߺÕƟ%?Y|ß?p"•°mi?Y|è4FGL J1737.3-3332¿ïãÁTÊ¥¿íã¨TáÚÀ8àòFÀ:vIë	Ï@¯'º@K•"d~?Åúq¶%Á[?Ú7ÖÛïTŒ@—›ý÷è@¨0‰à"ÿ?îØn¡Hdž¿Ù¾(Õ!°¿á¨ª®"Ó¿ës³‹³'	¿éFõŸ<q¿ïô™=SHUNASNone
?ŠGЁÈ,H?'f"~ʎí?ï–à½øßO?'f"~ʎí?į\}5
Z?Ìl­ç³üg?êÔ(಼©?Ìl­ç³üf?º…¡X /?¦¨PpX@?ì¼/KÔëú?¦¨PpX@? ÄQÈî`?ŒØ4ø?îó¾*ãq?ŒØ4ø4FGL J1737.6-2350¿ï	_½'@ÃNü½UaÀ9³ç't1*À;S~3Æ@m]–^%Ð@N€F}?ƾ—jjW?ÐÉD'@	ž³íQ@Ku&r°w¿æÞKòK?ïäÍ_ê2¿æ;À½Iø¿ä­Çüƒt¿ê2QáÊ	ú¿è
GŸUNASNone?͕M6§S~?ÉBï•EYž?蚬²V+!?ÉBï•EYŸ?Õ}Èv$v?Ôb2i«Oy?åAÄíÄö?Ôb2i«Oy?Ö/'œ'¹?»ÿS,×?äè6±¶£r?»ÿS,Ö?â/GuH#??»Bë&üý?Û¡qo¹?»Bë&üý4FGL J1738.1-2453¿êÅu™ÞU·@U.€F}À9&ÏEM+À;"£Ð_@)Ö=8ñ@.v»H@?Äx"%çEI?昚ËÈÀÏ@4‰¾ZCB@(ç-÷	?ïñýwŠ%?㲟YÌúð¿äpYߚYÞ¿ìÊXÿ°J¿ìb2Yï_Ÿ¿ê"tÔ¾2ÖUNASNone?|´ÄQ;4?¬õÿ?‹Á??ïƖwû]‰?¬õÿ?‹Á??‰ªÈ‡Ý'?¨Ì†Ö‰£?ï™TÝà‰¸?¨Ì†Ö‰£? ´ÒAE>€?"áÏP¥ËS?îô²Ûë¬?"áÏP¥ËS?^T'íU9?Hhê`™?ïðõÕ¶‰V?Hhê`™4FGL J1738.8-3241¿à)֘§$‰¿ç–Äg£}HÀ8ð"¿?EÀ:'o¶q@µ@uU«ÿ"@ZÊA¤æ?Ƒ®éŒöô?Õí3	AÈ!@	]®f°8B?ï‡îÁ"4€¿ïŊîÛëN?ïùvÿ:Þ"¿×¸o}f],¿ébü¹úb1¿ì¿Í_ï©Ç¿Çè5žrqbUNASNone?Nj.em¿\?ӀBbáæ?ê4f¤)?ӀBbáæ?ÀâÎuïHþ?ɺMK–'?ëÇLb"-Á?ɺMK–'?ÁºÊäš}?¬EÐæ‡Z?ë'MFÙz¢?¬EÐæ‡Z?†@!O]w?u0Z2±ø?ï¦ÿóz‰?u0Z2±ø4FGL J1739.1-1059¿Þe¦'¶Hž@%7â–é¼À9êuWšñˆÀ;r0˜N?ÿ@s¸7ê@P¸d_ûé?ØÐ\Ä|Y?á¸é‹It¾@7褙§Ü?ý¾îUÄE?ïþèÞ{Jú¿åöŸcÝõê¿â^þ]hã¿éùøuȿ뵃Úët¿äHŒ`ÌUNASNone?Ûý\&Ùn?͊îk]²?âQì"Hó?͊îk]±?ÐSâïåœî?ÐaªmŸ¾?çÖˆ
1‰?ÐaªmŸ¾?Ö¦\
&˜?·°âjG_þ?ä¬Ñüzì´?·°âjG_þ?±ž"26Xð?›"
ƒJƒ?íÌ-™¹4á?›"
ƒJƒ4FGL J1739.2-2717?éPx.fã@n½ÚÁ'À9UçòÛÀ:¿Véá@Y×p"½'@¶Iû̔™?ɟSÂÊÀX?×%àº?@Õ"~°	?öãXAµ'?ïGˆÒy¿å¥ƒb¯É¿á¡—)|Ñ¿è[@*<•¿é\žÊù¿ïÿÕ"[ʁUNASNone2FGL J1739.6-2726?£l¤õÙ[º?¥ïHêãW?îÉ5°¢jE?¥ïHêãW?¶[S¦Ô\-?Äø00²%?í4•‹%t{?Äø00²&?ÇÔc… Xp?°åKExç?ê
ç—éã?°åKExç?†þS¼Šò?sëêýoUë?櫓
Ô7?sëêýoUë4FGL J1739.3-2531¿á÷'ë%j¬@ÖûÅÜmÀ9ÚÖzËxÀ:ÉŇ^.@`æzGð@R):‹í	?ÀÄq‰…$m?ֈ$;ɄÄ@©(¿;ê'@‡rÑÙ¦û?ï÷º· "¿Þ}nàÞQ¯¿ã ³iNx3¿æ:½ …«¿íÍӒ¹«ˆ¿å¾Anµ?UNASNone?ƒÄ?®HÙ?®+¾BH?ﱈïFÜ?®+¾BH?¦VÇ=sqÅ?¼ÝvœØc!?Œ(Èã?¼ÝvœØc!?¢æ g"ì?"Ýbo<®Ù?îѝÿ‡±?"Ýbo<®Ú?¦JÍ
ê"?ˆüÅ m«?î›S/Q]Ø?ˆüÅ m«4FGL J1739.5-2929?è²À<¾×5?ëÌ¢q¯À9{'±HÀ;MøԒ"ì@5#ä`½/@$Þ˜¯?Ғ(ÁÀ)P?ïûB+ºü@úô­¼fM@«À›<8¿ïÿù³>†?ïÿ~'Ø	?´ÊÅ㤀¿ì51ÛD^Õ¿é8›‡°c
¿ïÿ+#š8üUNASNone	?'6¥ël¸?±`v+«P?ïnJ×(¤š?±`v+«P?'­øéË¢?˜ž†òMö?ïµHXÑx?˜ž†òMö?Àìø¤ç?ª¬ãæÇæ?ëÄÁÜû‡?ª¬ãæÇæ?a•l[â?RÔ÷Wq«?ïîðj"¤ý?RÔ÷Wq«4FGL J1739.7-2836?»Eõÿ@W?ôW½;_QŸÀ9Ë
F9 À;ºB¿˜0ä@ W·¡íP@i¾N"È?Òë=%Op?ïü ¨Â@(¸®1×?ý%@œ'hz¿ï÷&b?eF?ïölmçd(¿×Xï»^h¿Ø•o¾Sã,¿ïâa9Ö»?âN¦±\UNASNone	?}ì¶N7c¦?‰,ͳ€Ëô?ïÄ&"c'9?‰,ͳ€Ëô?ŠÄϒ™Žü?õ"æ\š?ï"ìÁµ™Ä?õ"æ\š?ÀQäj´	?«¬)ô.ž\?ëë†åxÒþ?«¬)ô.ž[?sƒKžð¤"?f'Lþ<Þ?ïØùh¶?f'Lþ<Þ4FGL J1740.1-1928?Û-'%¶@Œ¢:RÀ9E,Ñb¨À;ÀJÞJ¤@×ï½èƒb@#é Àiè?Ê©œ)&??ϲ?WÙ±@§~"ƒÖ@Árážëé?ïD8>4ï¿ãu]ÐÖ¿êøÛH"¿åŒ){D¿ïÿ>¤€}i¿ˆ5ø=œòUNASNone?áp!Yžº}?Îjûe5¼?ݽL‹?Îjûe5¼?ØJ#Ík¤?Ѩ0òÜy?ãÚîJ®?Ѩ0òÜy?Ýþ ?¹5 J˜J?áxxp€ð?¹5 J˜J?Ӕƒ.V'ž?²<í£ö©&?æ5¾hÔ·1?²<í£ö©&4FGL J1740.4-2850?ÌËÊ¥?ð
Ð"¢§À9†ñ·û"À:s¯þ_ìÐ@"ù‰@? §??Չüm¤HI?ØÈáè@
'h	ԕ@{……e…¿ïÿ2Döª?ïùÍKw͗¿ÚCC ¼
7¿â˜ÜP'`¿èÔ6¸ù±1¿ïûgêÊä•UNASNone?ӝ©ýÂ?ÊM]Ï m?æ1r+p ?ÊM]Ï n?ÓëT•GG¢?ÕJ³¢ݚ?æ
Uµ\\/?ÕJ³¢ݚ?àv=¥‡ã?µK¡ž©Äx?ß"´ñÖ9?µK¡ž©Äx?ä¥Oî]BÍ?¾Ù°5žsû?Öµ`#Ezg?¾Ù°5žsû4FGL J1740.6-3430¿îy3A¤hÀ5ĊÞìÀ9ùóEÀ:Í£ùZÊ@‰éOdl;@‰â¢!'˜?ÅÐ2²Ú³??Éédµy@ÿEÅÜï?ÿEù ½º¶?­ÇN¿èpöa7¿çBYì°¿äö¦_¥¬ø¿êõñ‰D·À¿ãĸ;SéUNASNone?ÊÞM4~?ÒÜîUÿR?éHl¼à2á?ÒÜîUÿR?âCâƒ=7?ÓîbÖë›?Ûx:ù…'Ç?ÓîbÖë›?Ùz´WAy?¸,¡g‡F?ãB¥Ô_sÄ?¸,¡g‡F?϶4'£Sž?°G{'ÑÙ?èrÛW+?°G{'ÑÙ4FGL J1740.7-6750?²|	½À2¯Ë':)ÇÀ:ƒž…'À<&c{Ð[@ÑA}£ÄÁ@°ÚB×%?ÂVûºKü?Ï¡Îò@úœ@"0{ÈÎ;@Všó
ú?ïý«&‰×…¿äØڌ¨ðO¿ì{¯¾Ÿ ¿åЭÍ-DÝ¿îDý[5¿ïÿߞ¶ŽóUNASNone3FGL J1740.8-6755?ê¾ƦÃ?Ãÿ¹Öm?ÅàådóÑ?Ãÿ¹Öm?æ¦É‹š#7?ÑBºý?Ò²lè˹?ÑBºý?å·Ü,"@Ç?·8ò&·S:?ԐG¦Ù~s?·8ò&·S:?âª
d—Çþ?·C…§©«d?Ú«ë6Ðp?·C…§©«d4FGL J1740.7-2640?Ë:Ý
ñEà@ÕinX£/À9¨‰ò\©NÀ;L'݃Ô@ð¿Îâ{¶@;½Ep?Ñú"å$²g?å7]ú14@‰0«½?þûþ0Gœ?ï«íßl¿⎧Þ*î¿Ø ­ŸŠõ<¿æŠw½¦¿¿ïÑdBSb¿ïäó¿ÕÃkUNASNone3FGL J1740.5-2642?'1PGçÃ?§•{ŠÌÀ?ïnu{õÀÃ?§•{ŠÌÀ?¢.ô×Ð
¶?¼IþZ<§w?îݲ'ÿ%?¼IþZ<§w?²ÎC£)ú? à	ž›'?í¦7‹šÝB? à	ž›?ƒ¬h²Üi–?j°:ä_È?ï±N]4ŽZ?j°:ä_È4FGL J1740.8-1832¿ÛôW;8¿1@kÓ^·E|À9ÌY…­S‹À;G¼PíX@´\®T@ƒ¦Mà?ÌûWϟ»?Ìs¾ÿÖ¤@öU&£ø@Dz"ø?í]ì_9K{¿Ó¥Üû(¿ã²°â
¡š¿éòÂ?U*¿ìÏ÷>^‡¿ïØÎÎ.̜UNASNone?æå¸Uéð9?Ȕ¤åË¥?Ò4T,Ž?Ȕ¤åË¥?貛£Ø_!?Î+ÅâÊÔå?Í5'pžƒ€?Î+ÅâÊÔå?åë~ëØD?µÐߋñÔG?Ô)(OÓy?µÐߋñÔH?è+Ëã('R?®TŠx'd?ÏPÐs]º¶?®TŠx'd
4FGL J1741.1-3328¿éšp²ÒáQ¿ù]ÄuqÀ9ÞL¸ÒDÀ;;3$º¼@§T ¾'v@$ÖÿU¶?ъ'¥aMù?âjd!èˆ@.;|­Ñ@ÍLVšÁb?Ü3ÿ`óµÅ¿Ì-ü}¦ü¿âԃ ±¿àIÓpóˆ¿ïÿý¡UûŠ?ïV⚔k\UNASNone?Á%ÉV¬?Ác(΀4?붍ªx[Õ?Ác(΀4?ÝÈïçèžÌ?ÕùLǘzÇ?áˆ°š?ÕùLǘzÇ?ÃÆ–•ô?°Ë™tėB?ëzÚZ»?°Ë™tėA?ÓQ£XË?ºxö¨5?æ}W@.Sš?ºxö¨54FGL J1741.3-3357¿îÿ—*éÏ¿ýÔlƒ¶ÙFÀ9Ä«^½ûyÀ:Ñ¢¡€è@ ¼Ü¥1þ@ø¼þ#@B–³5L?ãõ@‰]@ƒm¨z-@ã·­Uä
?ãÔ<ÞÓj¿îÿð:»?íD8>4ï¿ç.þúG¿ïóZ _†x?ïIÃ}˜²UNASNone?䕺û©N?Ò{°ÔâçK?×ÒԊ­d?Ò{°ÔâçJ?ãêÜõ7?؀#g¨Ì?Ø*Gãð'?؀#g¨Ì?á–ÐRâœ?¶&gûbHì?ÜÒ_Z;ôÈ?¶&gûbHì?ÒB"iO?Ô¹ÜՕc?æÞ¶xKX?Ô¹ÜՕc4FGL J1741.5-2344¿æ8?tû%<@òÒ»#WÀ9Ê:̄¨qÀ;´w K@3Æ̈́W¾@NˆÄ_@?ÑcáPè?Ý°Dä6@
Ž6A?û.'Å?ß?ÆßÅDd«?áÜlýÚ5ì¿ß±ÔÄ(¿ê[Ы~žl¿ï$ìH"É?ҟ.Äcœ²UNASNone	?ŠÝðèè¤?"\ߕAsš?>\^?"\ߕAsš?³ÃÒNøå?¾ÚJcà‰?퇅¶ ã\?¾ÚJcà‰?ºÛ£IY'w?¦t2ýÅ6¯?줋–ÔÏ°?¦t2ýÅ6®?¯øÉð܈$?"èÈ×ø[?îs`ò7}?"èÈ×øZ4FGL J1741.6-3917e?Û`6P
ð·ÀÞÉâ6Á]À6ücÔÀ:cã6îª@~ÇäیX@cyú—á3?˜2™sW;?‹Ë<Sî>·?òV¦4²4@ySÙFí?í¬œuìì'¿Ò¾ku™à¿áÁŸÂ¨†œ¿âCn9œ¿ä;˽Ù¿ÐiÕOçŸUNASNone3FGL J1748.5-3912?áä
Ž5w.?Ñáe¢®Ïd?Ü7ä㕤?Ñáe¢®Ïd?ëB
=†?ÐJ2iIç?Â÷çˍå?ÐJ2iIç?搓
§b?¼™%;£1?ÒÞÙëÚ±9?¼™%;£1?⋄öf`ƒ?ÁÂÝÇßç;?Úèö3>û?ÁÂÝÇßç;4FGL J1741.6-2730?çIŠKükH?÷âCV–åŠÀ9"uÝÒ®ŽÀ:ys›Ùú@ìØwÐÇ@Z5Ö|?Ë[›\<kì?ÚÓPtŒ™×@zÄÂ<P?éB‹êÂk¿ïÿÙÐs?ïÿÅè¬ý$¿æþýÝ;¿ëTGÛ`ä¿ìŽyP¨9¿ïÿgßbP­UNASNone?Ý-9rµA?ÙªævTÆÍ?á}écF¥`?ÙªævTÆÍ?¥x<w@Á?½•Î°1'Ç?î¯|8‹ô?½•Î°1'Ç?ijœè!—?¬"_®³ùÄ?êÓÅ÷»Z?¬"_®³ùÄ?Uj†&˜?Gx¿#90û?ïõJÀ<÷ì?Gx¿#90û4FGL J1742.0-3020?îòÞúZm¿±ƒÙÓ-©À8de+ÓÃÀ9 çJ&"¿@¤_ݶ)@ùGÏ¢j#?åãM"M2?Ò'5ø	'@ĸF-
û?þ FnÏ@š?éñUbˆ
{¿ÕAuÁ"I¬¿è±ÿ÷œ"0¿çù΍—,Ø¿ê«-u"›¿Ò¸`Jã(UNASNone?¶–7ÌÒa?ûX	Îß?í-9}%´?ûX	ÎÞ?ÐÔ¼(vô?Ñù')fv?çõ•¡ëĆ?Ñù')fv?ǐ¿²×'?¯'´@Þ#r?êÐJ:œ?¯'´@Þ#q?«ËÁªZ?¡tàᛮ:?îNÏCåZ?¡tàᛮ:4FGL J1742.5-2833¿Ð!¢å@ø?èÃoõPÀ8Â.jÑÀ:"P\8æ@i.r.E¹@(¤~Ïé¸?É@h:{üÑ?Õã*Ý#\&@qìb"IÏ?údDÊ=Ñ?é"L["e†¿Üaq¦3[¿ãONâ'/=¿èÄ1Bm7ç¿ï;_A"Û?ÑÂìúUNASNone?€ˆPæ8?'Ä 3éñ"?ï½ß¢¿ g?'Ä 3éñ"?½Eh<íçf?È3¶v,+ö?ìWRøbC?È3¶v,+÷?©¹Ä'K ‡?˜_ºà*±?îdc½‹Eø?˜_ºà*±?Šü¹¼!°?qW‡i^{?ï¹Ô
y?qW‡i^{4FGL J1742.8-2246?ÌÔv@è6;@
ñqýs]ÆÀ9°(¼·«ÓÀ;"bGóµ@Š•{&çË@;'÷
è÷?Ðl8¢Þ¼¹?ÛþÍzò@Ã#·;k@G91úÎé?ì«ÊÅ㤿á˜Tà'^¿â[óEÝYã¿ê*€Â2?¿îfd¸ç<»¿ï¸àâ"UNASNone?œŠÌêÚÂ?Ÿ¨9iX?縉©*?Ÿ¨9iX?ÀZhPª?ÃÕâ‰5Ë?ëéeëú•{?ÃÕâ‰5Ë?Â0ý²ã$5?®`&Bj?ësÀ"G6ó?®`&Bj?ÈØh	+?§Îõ?éÉþøeý´?§Îô4FGL J1743.0-3201?ßfÈä#·–¿òlÛzåylÀ8òñÝ'ŽÀ:i›€#¦Î@;MÄ®ñ@e|áÒîO?ÎÔ6SÏ
?Ñ!Œ!‹ëÜ@2€l'Ð@¤æ'™ð׿ïèùôMDV?ï,™†Nc:¿å!"dƒã¿æ1Iï7Zà¿ç~Ê-ëÌ¿ïÿþøþ"UNASNone?ÞOyx˜å?ÍãuÇoE?àØCC³x?ÍãuÇoE?Âɋ3®¯­?Ɋ"Á8ql?ëM3T?Ɋ"Á8ql?Ñå·|H¤¿?µ]CÞzP?ç
$AÛ­ ?µ]CÞzQ?ÄåÞè$4š?´ìøeào¿?êƈEöòÙ?´ìøeào¿4FGL J1743.1-3049c?ïùÃzÜ¿á"<5:tpÀ8®XŸÔF>À9ô"Ÿ^Õx@—'Ýè¨ö@@Ëò¤Î?ÊÈË5rþz?Лüà»Â@éý_;Ð@Ðyí¬Á?¿ïÒü›K ?ï½pŸM8¿çh*á«I¿ã'™îLÏ¿èõ¿¿óö\¿ïü\§ ÃZUNASNone1?®_N"S?É`"…Œ54?ë~h,^ì?É`"…Œ54?­,Š¼Yn'?¾F×ÜiÓí?î-7T:i?¾F×ÜiÓí?Èþㅏվ?­ãjåò#^?éÀGœ
?­ãjåò#^?ÀiÕ×b0¼?²Ìžö £¤?ë劊'sÑ?²Ìžö £¤4FGL J1743.4-3123?ì_&‡B¿ëú¾ï>'À8â֕£jÔÀ:@±NÂó@ 4^lFû@Ú½]Äu?ñ)ŸÖÊ|?ÎÕ< ˜@D¿ÒéF€@ßÿtißB¿×ù\B 6?ãsʒ`¿æ^B.ù"¿å#•0~M
¿ä{õO¡S¿ìä"CÆÿ-UNASNone?Ä© õ~¹?Æâcm,ï•?êÕ·ÿ R?Æâcm,ï•?Íðæ€/D{?Ò¾Áŧ®?èƒÆ_ô.á?Ò¾Áŧ®?؁¹ˆ–‰q?º=ÔGGMw?ã¿#;´»H?º=ÔGGMw?ÞÖ»
mÈÐ?Å`³ºŸÇ?à"¢yI˜?Å`³ºŸÇ4FGL J1743.4-3406¿î_qõ]ÀlZßI§À:ZKÄ#°ßÀ;®
9>åï@áÑcµ\@Â=&Ñü?Øéq}ñg?ãÜ|m8è@y‡Æ2~Ø?óï•!îZ¿è$EÅ.î?ãü`£®ÆR¿Ï|èˆêö¿åÍ´Þïd&¿êŸÐJ/Îû¿å¾§°³'UNASNone?›ˆ7áoX?©‡!"Y?ï#¿6@ô…?©‡!"[?ΰ;¿f¢"?Ðñú藿þ?èSñ&W[?Ðñú藿þ?ē¦Ok6à?­2í÷'óÿ?êÛl%2H?­2í÷'óÿ?ƒèÞ)B~K?p(è¾+j?ï°\‡Zö?p(è¾+j4FGL J1743.4-2406¿çÛyo"ýŠ@yߖÓìÀ9¢"'¡WÔÀ:èñ«©f–@ê£q^¼ú@Aë¾íç?Ê{‰¹&Ò¨?Ïe7ýO1@EÇ
âA?ÿNç àö%?íQŸ?ûs¿çzä7Lh¿èZ<ŒxHç¿à"à4ˆÉ¿ïÿþøþ"?ã8}àU•´UNASNone?Ü´_c
3/?Í1ô Åßá?á¥ÐNzæh?Í1ô Åßá?Ý*$ôãRd?Õ§RŸÕ?áj텎VÍ?Õ§RŸÕ?Ùµ.Ååµ?·!"£ŽX\?ã%h±
&?·!"£ŽX\?ÜmÑ8©7?¼V,Ú&¡{?áÉcó«d?¼V,Ú&¡{4FGL J1743.6-3341¿èåxKMÀÝ!ê6À9•$Š#À;‰¾ZCB@ m™Y_@õ~íEé?è&ûíKÈU?È/«©¼|s@øZðŸ@[2\sž]?ÁHç$'Ú³?ènæ4'¿Ëñ.Uþº0¿ä5çéóN¿ævñ~\ý1¿éIO4¹ÀUNASNone?ݐyӄpj?Ð*h|×?á7Ã=ÇË?Ð*h|×?íå7¯?ÈrÞIóå?·p×c~B‰?ÈrÞIóå?ç%*š‡­¸?¹Y\^Bï9?ѵªÊð¤?¹Y\^Bï9?é>j±š)?µûB?ÊU9—\?µûB4FGL J1743.7-4321¿Ó2? •Á–Àª#žj¹²À9ËÍiª¾…À;òHv'VÕ@äÖÈN7ñ@^½$¹?Á–I˜z_Ã?ádv6¾/@9ßÞè@Ž÷Õ:?豈bîпšàRe¨{_¿ÞƧCÑ;¿éûß¿˜±½¿ïցz"ð¿í¤{	‹™ýUNASNone?Î.*Ž?²¯|tC§?ïÀc£Éªã?²¯|tC§?˜øš^UÑ? _¬éŒ_í?ï8;/5
R? _¬éŒ_í?Ž: J¥R?zB¤˜rä?Õl?zB¤˜rß?™ab}^J?|Œû¤¾»?ï4÷,ì?|Œû¤¾»4FGL J1743.8-3143?è#5ÕMá¿ò:øúRAÀ9['IWbÀ: ¼X
ƒ@!]úŒÎ…	@Õ¼{`É?É2ØÅS†»?Ÿ!N%Ê6g?ße)ÛÃP@Uvꚿí!ñÂO›I¿ž-QûRú¬?è'_³Ä¾¿å'§¢pØ°¿è<Èk.L¿À•¸#®UNASNone?è$.æð³h?Ét¶¦ÜÀî?ÏoDd=2`?Ét¶¦ÜÀî?îŽ(­°Âõ?à %ŠfG?§u$óд?à %ŠfG?ç[SU/¥?»1þ4|9?ÑIYUÙ ¶?»1þ4|9?í"Ïó:¨?¨#Òۜ?³a€g&*Æ?¨#Òۛ4FGL J1743.9-3539¿ã%—Ô‡N'À	¥%1À9Í:óñÔÄÀ;bʤÔ`?@1¡¸¡ó@‰ÂÁ±Ø?χ?ÏÏ?ä	pA0¡Þ@+vö×bR?ûç­ôDŠô¿ëÝâ¾ü˜?ï2«M÷¿éÂ!øù&¿é©yámm¿ïüpßFI¿è!8>µÈNUNASNone?ØTÛK:?ÐpÎZ>?ãÿvՒZb?ÐpÎZ>?ÕxZut'\?ÓÖùê
·¹?åCÒÅE¶Ò?ÓÖùê
·¹?Ó<`3¶M:?¶Ë×ÄÒW?æaÏæ$Ùb?¶Ë×ÄÒW?"*};ž1?'DnrÿŸ¬?ï[–¬#?'DnrÿŸ«4FGL J1744.0-2504¿ïù§—½–%@ƒá†˜5À9BÍl.ýDÀ:¨ÙRîº@¦9kÜr@§"~§¥Ì?ÌÓ÷8†.X?Í>@,•à@²Å"Ùîô?ð±BøΊ?êÑr¹[¿ç¡ŒâÑñпèÉaÔ¿èç¤T¿¿éñþë-
$¿ðUNASNone3FGL J1744.5-2506?à­Q	c ?ÐûÈE¿:I?Þ¥]í9¿Ä?ÐûÈE¿:I?ÐäçG7Ý?Ó0ÀK½Ã!?獌w\d?Ó0ÀK½Ã!?Úã\(º¨?·Ä#Š³?âŽQ뢸+?·Ä#Š³?¤
Wͳ>5?'<m©¨à?î¿Zƒ$Ì?'<m©¨à4FGL J1744.0-1311?æïÐ!ÉËf@ çqdÇ)öÀ9®ù–Ys9À;Tpš@(żãÊ@íqåöi~?À‡kŸ‹K?Ñ"ÌHBŽñ@PLýߔP@‹È>?ïÿº*2Ùq¿À¿1ÄPÉ¿àÖŸd´µ¿áê2¾™-c¿ëÃé.,c5¿ïÿŲýîUNASNone3FGL J1743.9-1310?µ¢|ÅV?²¡InëÌ?íK°g]Õ0?²¡InëÌ?¾Áùë²AÖ?ž‡A°L?ì'À‰·Å?ž‡A°L?º€ÍWZ®;?ªÑ󮋧Ù?ì¯æUª9?ªÑ󮋧Ù?Ïo1\ð,?ªÒùæÄÐ?è$3¨ÿÃö?ªÒùæÄÐ4FGL J1744.7-1557?ˆ>"AÐ@Ÿ§¨PÂÀ9ybA=·ñÀ;m§<ð@"ᷕƒ@ìC9+?½º›ÇÇ)u?ÏõðÝx@®@Îގ–0?übE1¸^×?ïÏXBaNz¿ÝqÍbHõg¿æ(Æ}}YG¿â£Å&p­¿íPA`ó`¿í±P$QïUNASNone3FGL J1744.8-1557?R:;câÎ?©¢FVˉ?pu?©¢FVˉ?£oRgªY"?°†ûkm?îÉ
مZg?°†ûkm?¿ÒtÄeÉD?©P›wE³(?ì±gsF×?©P›wE³'?ªC›ž¨A´?‹˜"¬ÙU&?î[ÆF{å?‹˜"¬ÙU&4FGL J1744.9-3322¿ÚåN¢r"ÀÎú¤vlÀ9x ]Øù+À;!ÖÜñ?@ES#há@Nc¥ÁÆ	?Æe
›º[0?ÝĄ^žò@ÞÔI˜Ð?þ§/ç¤>Ž?î&mó"¡ë¿äu°»õ4¿×Yӟпèi¢#¿ìpâ ôÈ¿ïôè_Op×UNASNone?{ P«"V-?xÂY€çâ?ïÉ¿^¨ÙT?xÂY€çâ?·¡.F•Ù?ÄS'ÒL?íÚ<·-F?ÄS'ÒL?¥åW–}	?š¦¹°=¤?‡&˜/?š¦¹°=¥?‰@ç!.'"?qMØSÁš??ïšüc{Eö?qMØSÁš>4FGL J1744.9-2153?î#œ´bÌê@_j^B«vÀ9•
ÿÀ;o#¤I÷@0–¤Ç @DeÀN9I?ÐҋÿH?ϒ¤g"@í¶^Ì>2@GºÔ§¸¿ënM?ùÀ ?ëÑÇ]w)'¿âü¯þàÆ)¿èêÂKiŠÞ¿æa@AŽ•¯¿æžë/ŽcUNASNone?רs(X>ô?ÌâNˆ;=l?ä+ÆkÓà†?ÌâNˆ;=l?ÖÃ2•6‡?ҍªߕø?äžfµdø;?ҍªߕø?Ù
¿O¤?ºŒ7¹h?ãz |Øq/?ºŒ7¹i?ÙɸQæÊ?¼<kßWe?ã#×vŒ›?¼<kßWe4FGL J1745.3+2338¿âëaíQ@8~
"¾@BÀ:T3‹GÇ?À<*»êý9|@Mheïóî@`êžnëp?»
míq¼¿·&¨
u¤È?÷¸)W^Í?üàcR4ֿ°£?4É¿åmbÙéë¿ìŠtBrq¿å™Þ"Û¿è;?Á¶ï?âÊC…ÎUNASNone2FGL J1746.0+2316?ï‹)ˆºÈ?OO™¯?5ûÑN?OO™¯?îJ°N·øO?ºà	ÎG7?«Tû€{?ºà	ÎG6?îÄ^ñE‡¨?—•ì!û?£º맅‡?—•ì!ý?îÛ~XÊK?"7IÓ§ÊÚ?¢Hs[Nü?"7IÓ§ÊÛ4FGL J1745.5-2249?Þ÷t¡ù*¯@	šxš:À9ÙéðÀ:³m—³Œ@_#·SÊ@P:ÅΫÊ?Óµ^>J?à™ØZiÙ@	z™ÄaÄ@@d"µÔ㝿ï·]d_%*?ïñ"Á"g¿ëMa²¢¿ð?ïÿû-2h2¿ïí}±«´UNASNone3FGL J1744.7-2252?ìh'Ÿ>^P?Ŭøm¶¹?¼»k

‡?Ŭøm¶¹?Ýp¢´I{j?ØúS.`Wb?áG®¥ÛBJ?ØúS.`Wb?Ù×1…H?ºÊíX7º?ãw"g1=\?ºÊíX7»?éáïZ›?Åý¤c ?ː{°B•–?Åý¤c 4FGL J1745.6-3626¿ÄŒÛ‹ÄnÀA&:ý,À9Y©mL3µÀ;KkÊSuÉ@}Š/™J¿@|­€k`?Ŧd׍?Òåí/Bä@…»¾‡¬?ÿ¡?¸§¦Î?ï¤Î(™Ò¿éšÌ¿¶¹»¿ã¥@@âÉ8¿ânøÁG]¿ï¡‰R#¹?ãJò|‰¾UNASNone?ÕÅ 0k0r?ÈêVÛ\\ê?åoçÊgÇ?ÈêVÛ\\ê?ä3>þ?Ô+6¸¹7g?×ùϘł?Ô+6¸¹7g?Ùù?Û°d?¸6'&8Á\?ã`z'Ï?¸6'&8Á]?ÜBN,iZ?·ÖþGº%Y?áÞØéËS?·ÖþGº%Y4FGL J1745.6-3145?ë`U8°yd¿÷¨Ã ¢7À9·k;¸=À:׆¾Ë'J@‹øyMô«@Qw~¼ž?Í7•˜ƒ%?ÙjÈ˶L@7Lg"t@mºB±€?çÇ_¥'(¿á£tä®k¿â(Ùþc´¿å\ƒÄE>ο煇"Ý—ö¿ïÿÓà<k@UNASNone?¾­;ݦ^?»«ÌÆËç?ì*X"K4.?»«ÌÆËè?ÔÒűӘm?Ӝb¯Óù?喝'3Ê?Ӝb¯Óù?ÔÑýÑ[øú?·¤'"Ñæ¼?å—Rƒ?·¤'"Ñæ¼?ÇšóŒ?®Õ¦ÿ}A®?ê8ÙxCß?®Õ¦ÿ}A®4FGL J1745.8-3028e?ëŽÂK^]¿êÈè§æ›À6ŒŽž"Ô^À9¡PþU0@ lÒ³k§Ä@æJ>ès? kæ­ôo~?˜ëã=|?õ×??ñ/Q|I}?ïIše]R¿à
Õç'Áæ¿â#揲¿å$;´4ç¿âÀœ<âž¿ÝŽèÑQ­UNASNone3FGL J1745.1-3011?ÙÕWn²`?Ò¢.sùt?ãTH¦ýÐ?Ò¢.sùt?Ԛ$R±?×¢B.²
?å²íôÖ§p?×¢B.²
?âi«Ã=?¾øWh?Úßé,¨yƒ?¾øWh?›Â<|¬?—úJ¶ã©?ï')î|?—úJ¶ã©4FGL J1746.1-2541¿îŽÖO1?ùMë­òíÀ91áìï'À:ö"o³í@n‰šs@1*å†×ö?г ž†~?Ñ!
Gé#@
MFðP?è
ۉº9³?ï±K(¿åV…í	¿åǐbcL¿ç§/^½O¬¿ë!¿îB¿ðUNASNone?潬ãŸN?Ѥ.Ë9¾?ÓԄ¦8Ád?Ѥ.Ë9¾?ÁÚ¦(ηs?Íipτû?ë‰VuÌR#?Íipτû?Ôːտ?·BÍÔö0e?åš7• rõ?·BÍÔö0e?pÔOíR±u?aÖÚG°Çü?ïÞW`%Zž?aÖÚG°Çý4FGL J1746.5-2019?×ùG&@pý@._¢ýÆjÀ9l~|áœÀ:Ø¢xelk@µètž›@.ƒþý¡?ÒVñé¼Çœ?іé;ƒ)@	±ÕšÑ§þ@€¹xÝ?á7¢~D©}¿¿K¾ß8¿êTݧæcw¿å›ã@+¿!¿èSZ_òÙÒ¿æìa¢—oUNASNone?ÖþméÑ?ÏUs$ä?ä€É}r?ÏUs$ã?Õµâ°ó¥¦?ҕ†ÍÏ?å%§†--?ҕ†ÍÏ?ãM¬ÒÂ#'?¶ËZ_|Å?Ùd¦Z{¹³?¶ËZ_|Ä?ÛÆQ™k?¹<$ÝJ5Å?â×3J~u?¹<$ÝJ5Æ4FGL J1747.0-3505¿ïΞt&À³~²†fÀ9;AÖNVÀ:ð~gäì@¨ç ÐH@€"Ýz™ú?Òý¤Ûìû@?àž«QR+@3¡/?ÿ¸†^©X©?î̎^''·¿ÓrP¿á¿ã@Š3Ë	¿ë©Ùîm¿èˆ"#8m¿æ)7fžšŠUNASNone3FGL J1747.0-3506?—óÂoK&º?±žVåã6\?ï@a셦Ê?±žVåã6]?¤HyËÍOJ?µ§Ì§N…?î»xcC+?µ§Ì§N…?ÃdÀ<
j?°Sl u<?ë&Ïðü¾e?°Sl u<?V2«—ÒÅ?L*&³AþX?ïôæô*4?L*&³AþW4FGL J1747.6+0324¿îü"1"J@/{À6âëÀ9®Hn-ÛÀ;¶·»*ä@™Km¼›ý@Λ¤5Õ?½µnryo?Ê0¬O·x@
"­äª9$?ÿlyöf#K?È{ø^v¿â_N_¤¿à©áæ9…]¿ÞZ؍u¿í2wKø¿ïÿ⾦™\UNASNone3FGL J1747.3+0324?ÌXá/u¡q?Ä="á w$?èéÇ´"—¤?Ä="á w$?ÐùK?Íþv-N'±?çñ|úZB?Íþv-N'±?Õª»–ÞÛò?ºqÅÎ?å*¢4'?ºqÅÎ?ÛЋOÈÔÇ?±^twÐÑ?âºX•ž?±^twÐÑ4FGL J1747.7-2141?û¾	¹@
½¿cíÀ:ÅÛAÖÀ:õ‹QØ9è@ð_ŸLáÛ@èIåý{?Ô$yÜåɞ?ÀmŸ*R9?ðfÝR@ª¯³…S¿Ð€¡öµT¿èù›ÍP€K¿æöJßø"¼¿ì7ûþé¿Ê$xs'.¿ïõŸŸ1öUNASNone?ï'^D?™9;ÅÑd?Œ:6=(o?™9;ÅÑd?ï*0û4á'?¶ÑW×ÁÉñ?š¹à™cÍ×?¶ÑW×ÁÉñ?ìEiɬc?­…@Þ‡a?½Ô±²œãƒ?­…@Þ‡`?ïƒ,¡2XF?…v2ÊjðF?4׳iîh?…v2ÊjðE4FGL J1747.8-0316¿ê±ü,>¬@)f+®´À:ÕõbLMÀ<
Ê7Ǫ@!êK¸»?ýÓ
ÔoX?ÓÞõCc'?Ó¬¹1–?ùC,Tò œ?õ`¹ÿÉ¿ïùæuë>¨?íK@š$?è6x—ÁRE?à'՟Ú%¿ç½ûm#D¿ä÷ëÿ—û4UNASNone?ïµB—Ør°?Sf¶©?'¯Z	ãT?Sf¶¨?î öÙÀ"?¾~UO&G?¥ð'oöÏ?¾~UO&G?í‰yʤ=?£
xÁè•[?³´7qªÞ?£
xÁè•\?ë;Aݼ?´^,þAó]?Êø‹­?´^,þAó]4FGL J1747.8-3006?ÜÈP©Ù•œ¿ð}'@.Ä9À9ÚZgT£À;‡º.d—@ Îî™Ñ!ñ@$½Ÿ2_Ï?×}Îâћê?ïRú®‡gh@ž–›¸WË@¤öí1Ç"¿ïã%Ô¥ß"?ïgòPµû¿Ø–8ù€Š¿"Ÿ\èä0¿ë¹ýßÒ¿î女©UNASNone?·sÛ¨°¨û?¼–L>ì¹±?í"Šéêá?¼–L>ì¹±?«í®!L?¿x#IsØ×?îA%½ï?¿x#IsØØ?ØÉ´ÑûK*?¸Iÿ
úÇ?ã›%—Zj?¸Iÿ
úÇ?´w%ghÜø?¨ÒŸ¢<?íqSä`?¨ÒŸ¢<4FGL J1747.8-1827¿ïƒìHŒÏ@æ¢nTqqÀ:Qè·§À;Ê×)G!'@Ÿ6çrÀ@8âºtÛt?×¹vCS;ç?ï.À½të@ß«ºbg@é—M¹ò*¿ïÿ*b{ö?ïûd;¿êPëHD½¿äeÛ&+ã´¿ïÿÿÊPË?ïþá˜á¹UNASNone?¿},œiû?ƐíI)?ìZlrÝ!?ƐíI)?¹Ÿu^0?ÇÖÃC_Í?ìÐT:?ÇÖÃC_Í?ÖÄ=¶9{?·Äó-/2?äá$ãBq?·Äó-/2?½>Š)wB±?®2Éh·ë?ìX.ºÑª?®2Éh·ë4FGL J1747.9-3224?äø]å[ãÀÔèÅP׉À:¾¶‰"iÀ;?"øS@+ƒ«›¤·@Ãf½Ì?ÑØýݐêI?Ûnàˆksì@	ÉrŠar@€Ì T‰D?ïðvŠ ØR¿çu5×RaÍ?˜ y
'¿ã5"÷{Í¿êDFwÜ¿ïÿüÚ±'ÞUNASNone?ä0ýí%"?Ì
À?ןÞ%´Ú?Ì
À?å͜lk-š?Óu©ë\¢'?ÔdÇ')¤Í?Óu©ë\¢'?ÚÝЅ'šÝ?¹QD.gÌÐ?â'½l2'?¹QD.gÌÐ?ßG"(û`H?¸"e®?à\në'OÜ?¸"e®4FGL J1748.2-1942¿Öæ½6Ã@ålÖÂðÀ9
‹ýáÀ;>–•[$@b'AcL«@-¢ÝåùÄ?ş£†ØL?¿=f<õÔ®?üT\É.²›?úÉ·0Ù;Æ?퍝aûÁ¿àfêþ<¿äSÇÝúœ"¿êHÒ!Š_¿Úý[?Á¶ï¿åës¶±•UNASNone?ì¼d¿ˆî?·ñ¥ånÇ?ºÛò¸?·ñ¥ånÇ?äéìغD?ÑH`!?Ö-æ&N‹z?ÑH`!?ëÌKp8?±[½¸!?ÃÌÎÒ>?±[½¸!?ä'Ö{?·ÏXì$"±?×±ÖSßÇ
?·ÏXì$"±4FGL J1748.3-2906?ïŒïí(¿ãW;P8&¸À8+Apã—êÀ9Äöæ{Ê|@­õ«"A;@ý%àdYF?¿Ÿ©¾×ý?ԉƒâM<Ÿ@E¿9fS?üóâہñ\?ŃÁ–ò,?â<AßÉSÆ¿áÿÊñ*z'¿åž¯ƒêY¿ë˜ÂÚÄ¿ïÿÙi"A'UNASNone?¡å]Žv›/?Äå2'Ææd?îáª'–N?Äå2'Ææd?…ô61™è¶?™•¥¨¶é‰?ï¨/'9˜\?™•¥¨¶é‰?'¤<?C¬?‰¡»»¨Ù¡?ïjÞ=â?‰¡»»¨Ù ?U0XÜÀ7?GË5ÓÕ×?ïõgÓó ?GË5ÓÕ×4FGL J1748.4+1601¿ïÍÒÆaê@4û3ÚøßzÀ:ÐðŽrôêÀ<K¡qÕ/r@Ɛ'ˆ(-@?']<9?ÒJ2žb×?Ù¦%ä@0ó@Àa"V!@Gœ¡¶Ê?émjf¦'G?ïý%?T©¦¿ç	¦ý…Qc¿äX,²²%¿ïþ\ý1§¿"É*gøUUNASNone?ëùô{‹?½ˆ–LM™?À.ÁÑþ?½ˆ–LM™?åa¼ƒŸ,Ò?Ò"d^ôêÛ?Õ<†øÁ¦\?Ò"d^ôêÛ?ézòé}?®È…±2ïÝ?Ê5¼[®
?®È…±2ïÞ?橇Pf'?¶ÊmÏ÷{?Ò­Ôñ_3´?¶ÊmÏ÷z4FGL J1749.0-2119?颢éÃæv@
0d‰Ø[À9…
a'ÏÀ:­y×\rÈ@»˜•±ƒ@<ó~}×?ÓÂìCŠ™L?ß¡2À¹o@ÛÐüv<?übJG¡Õ'¿à+"H×à¿âØÂ!y¿ëðÞ¤æ¿ëF®::Žq¿àÿñ½GÌ¿ïãtÿ†]}UNASNone?å'å"¾Ú\?Ðæz~ÞKþ?Õ°5º'KH?Ðæz~ÞKþ?āþ"é9?ËÍ¢œ?êà€wE²?ËÍ¢›?ÙTmyc?¼ûƒþœT?ãUÉC9Ny?¼ûƒþœU?´P˜-¨7?ªÂÚïOX?íuüŒúJú?ªÂÚïOX4FGL J1749.6-3143c?ïã\]êÀn²Ð¢DcÀ:ÔK3ÛÀ<j¦gv@`ÆyvŽ}@åF
¦L0?Ðô»¾²'Ê?ïr7Pþ@ù?R%g@=‰"~¿Öy>‡$L?ï5ÞUö¿¹_ò.+¿ÜB‡d
¿ïßëìd?ê:#aÔÜUNASNone2FGL J1749.7-3134c ?­ýÚû´.?¶ÑH3³"?î "_ÀD½?¶ÑH3³"?¾7òøÌ`?ÉÜ0÷ˆÔ?ì9 æ|"?ÉÜ0÷ˆÔ?Àt!·ÍôA?©Ééãgtf?ëâ÷''ð?©Ééãgtf?ª7®÷6¾Ë?œÈº=?î\…Œ"?œÈº=4FGL J1749.8-0303¿à"ˆˆ@‡S@(q[Ývh<À9.¨mqóbÀ;\ý#¬­s@·"CñòK@FC´g?¸¥.ßL½Y?Ñv°@O%'@}"Ó8÷˜@2A~$ž?ﹺAn_¿á"¹"K‰¿æŠ"XŸÔ¿çu –
¿ïþ@½Šd¿ïç0ž-}UNASNone3FGL J1749.7-0305?àÓE«`†?˝n'¡à?ÞYuÒ©>ó?˝n'¡à?¹¿ø]²l{?ÈŒz#ú?ìÈôI²q?ÈŒz#ú?ØÄ×Íh?´ÎCŠˆ½?㝔xËý?´ÎCŠˆ½?ÄrP¹õÔ®?¡ûþ'M?êãkтŠÕ?¡ûþ'M4FGL J1750.0-3849?ï¿ÿª¥…³Àz)³únÀ:FdÆSÀ<ø´²#Ô@ÝâF܈W@Xô›Gïƒ?ËJ}|­z¢?êÁLÁN¿V@ÍäKjb@šº†N8G?ìP¾´[<¿ÛÝÉtR¸4¿àÃ?O¡(¿ëúç\›Š¿ïþ'Ý¿áŠ¯ñʳUNASNone?™yÁòZ½®?°#9¢e¾Ç?ï41ðm*?°#9¢e¾Ç?ŸP72%P??ªt¾íÄ¡è?ï~FnÕ~?ªt¾íÄ¡è?´åkuYáö?£´ƒÛëè?ícR'TÃÂ?£´ƒÛëç?Œ©	ZÞ~?vœhÁWò?ïå[ڔ‡?vœhÁWò4FGL J1750.0-3347¿Î׀6ð'À
™ÔttFÀ9Åét£@À;HöHÇ/@\ÜÇÁ @}N?(3ü?Ëøg…JW<?ÑUA8Úg@†&oÖQ±@¿"²²oS?ïüë¾TŽù¿è–µ¹ŠÑ¿É!"ßù$o¿åÞjNRsj¿é±y?%3¿ä¢W
--UNASNone	?è±3PÖî?ÇbáËL¤ê?Í;2½ˆ¤G?ÇbáËL¤é?ì¼eñÇÉu?őU%
¬?ºÐqÁ´X?őU%
¬?å±õƒ¬?·{Z*ê˜Þ?ÕñÀœø¨?·{Z*ê˜Þ?é$¥Ç:æ¸?ªƒ×ñ¼p?Ëmhãe?ªƒ×ñ¼p4FGL J1750.4-1721¿ÞGž_ï@	$kðÀ:òÕuûÀ;¶၏¸@¤X[¶µ@ 6^`Þg?ÉϚ‡€<{?×ý¾¼éªÔ@»A®@ñ@…šPΤ"?îðÉ@Ñ+¿ãÁ9»ãp}¿â=d_%)…¿è_‹*ì¿ïÿÿ" 5•?ïÿû-2h2UNASNone?Ö͵7§½s?ˈeÓký?ä™%d,!G?ˈeÓký?ÖgƒçÍ?Óxd¾6ëÛ?äÌ>1??Óxd¾6ëÛ?ÒPA3*¾?µË3ðÛ?æ×ßfjö¢?µË3ðÚ?Ù+»¹™Y?»ÇÃ3¼<Š?ãjp"#3T?»ÇÃ3¼<‰4FGL J1750.6-1906¿íkcÏØ%W@Q€Ø´À9lm½r¼¶À;	:×lc@"!"9Å@þ7"«üs?É·¸=žœ
?ÌϞxÑx@}£!ØG?÷ô›ï	?ì4јäh¿ä×ø¿Äс¿é8Ï>ìúÀ¿ã»?Ï¿ì^ý¼Xá¿ïý‡ŸñøUUNASNone?ÆÔ¼þª®?¼=‹P71?êJÐû@UT?¼=‹P71?¹úÅ8Êêh?ÂÿèͲÌË?ìÀ§X梲?ÂÿèͲÌË?×ØÙt9?¹"âsO?ä"Eôpâ?¹"âsO?©Éí5džŸ?'´3P£?îca,£‡–?'´3P£4FGL J1750.8-4405¿ÓCè*D°­À!Jæ…Ûv´À:gþÓ°ÝÀ;àZ›W	@öä¡TÎä@Ò	Å{Ÿ´?Ðúk _pÿ?Ú?B5.µö@ž$»¡+^?ú¸`ygu¿Ø-³Âd¾ñ?ïÏ¡ýÁ6¿ÑµA*l»¿ä;ñb®K¿ïÿà?Æ>"?ïúñm–UNASNone?æ[XJÁ?Èímܯp?Ó÷IßOj?Èímܯp?çÿ|ê÷…y?ÐÉj²å&n?Ð*õ
?ÐÉj²å&n?â>ŸG†è?¸)Ðy]Ö?ۂÁpäò/?¸)Ðy]Ö?à4	+w?¼XÙúAìx?ߗùùí©?¼XÙúAìx4FGL J1750.8-1246¿Ù2"uÌT@å$9›,AÀ:€T–ZIøÀ;©Äÿxñƒ@2ް@º<÷T?ÖVԍ‹n^?ã<¥7\ @"ª^ã»&?÷y¿¹†?ïÿÁ¡u†¿à}i[
¿Ø|1©Æ7‡¿å@p"|ח¿ïì[rí]f¿ïäu_þmYUNASNone?×h¸<µ!?ΟÃ$'.?äK£á¥os?ΟÃ$'.?Ѓºº
zž?э3›'?ç¾"¢ú²?э3›'?Ô¥YþG?¶àqž‡ÏÔ?å­S€ö]?¶àqž‡ÏÓ?°çêø0?"ïqÑ:?íüã ü?"ïqÑ:4FGL J1750.9-3301?ß|0®"ó À¡f>ù:À9º:NÀ;9=e¼{@Æ<幃@–õw/?Éú»¡ w?ƹ«R5Ø?þ%½ÿªo«@v:2€Û³¿ë<":µ´?ïñ@x@.¿æo;At"|¿äf†a®pÁ¿è›
²ái¿ä5M>ÍPUNASNone?é3^‡}Né?Nj¶ÎM?Ë2…â
Ä[?Nj¶ÎM?ìÕÍR—æ?ÊsM 
ñ°?¿ÙQ•k@Ò?ÊsM 
ñ°?çh/µú.˜?¼­Æ‹‡:?Ñ/ "¢Ñ?¼­Æ‹‡9?êf¾.ƒð?±Èm¥ØIÜ?Æe›Eð??±Èm¥ØIÜ4FGL J1750.9-2655¿åý{ëð?"¤ßʚ1À9)LøW>À:ªo ¡Ë—@Ýèuõ¥‰?ÿe©Oð?Ϧ-ü'6?áÅ»ámÛ@ÛxFbºà?üAmwþ?ïþµ}$îÍ?è­½¨l›4¿Öàæ?³¢¿ìzD5ë¿è¥Ùä"s¿î|¯þàÆ)UNASNone
?Ȗæ‹Xq?Æ¢tîvC?éÚF]9©ã?Æ¢tîvC?¾ZÒï<Nm?ÉÿO5ço«?ì4¥¢v3?ÉÿO5ço¬?ËÅpÎRx?±%áMQÅç?é£Ìk|á?±%áMQÅç?±â>þæç?˜$ë®[¯³?íø >#?˜$ë®[¯´4FGL J1751.1-3455¿ì­ó·J–ÀUiR‹¾À9ø'õ:ª À;i²KAFò@_fPÁäf@ÿ#a.?Ê´®ÈÕÇG?¶)vpõ‹ˆ?ñÛCˆ×?÷WdZÈx?ïŒ$Ñp |¿ÞâšÎÍÙ¿ì{´ÚgÀ¿ÔBe"oä¿ê±ó˜°Ý¿ðUNASNone?ï©ñ¸ºð?Ñ‡Ô?…ƒ'ÑCÜ
?Ñ‡Õ?î9}J'¤?ºASw?¬h+W&å½?ºASw?ëÇîk¸?©£0Q(?ÀàFS¡ã?©£0Q(?è.ÈQ2ÿÞ?±¥KAÎU?ÏDÞ»4‡?±¥KAÎU4FGL J1751.1+0109¿ÑÏ}T€éä@+ÙØ@žUÁÀ:E,YûÀ;°"L*zþ@ë"Ò/bC@œ'W…øÓ?Ԁr¡]2`?è*±^Ý0@Yàâi?ùøYMN<y¿åÚâ9E›ì¿Ý¿‹0JJ§¿èK"¾h…û¿ìœ.¿†S¿ÞÞõöÕ_¿ïó"כ\èUNASNone?Öú`‹ŸÙ?ÎlZvþ?ä'ùϺ0?ÎlZvý?Õ±tƒQž[?ÓpÙàí{Y?å'E¾W0Ò?ÓpÙàí{Y?Ü4è}•?¹¯^¾?áå‹òA5u?¹¯^¾?Á͙ÂÐà?´íl`§—ë?댙KÇù?´íl`§—ë4FGL J1752.0+3606?à3£±@:î®ÀrKwÀ;nƒÚ³ìÀ<ÎI2xù@ ICF¦­~?þâ¿b€þ˜?ÐÂHyìU(?Â+ÍxÄ6ü?ó¨(Ãm¨z@»Ã>-¸?ېR.9#? El¿ÐZakTã¿È(aP¿íXØãÀ¯?À[˜·§wUNASNone?ïé¥#·g`?c'Í:/"ó?fZÜH˜Ÿ?c'Í:/"ô?ïúՈixç?jê$A€]?D©ÞZb*?jê$A€]?ïT@în?íN
Û¶G?•wâ?-ô?íN
Û¶H?﯇Iã™?tÜˋæ?"8ž-‡Î?tÜˋä4FGL J1752.3-2914?ìR×Ú¼¿öž²r®sEÀ93âÏòÀ:N:†
˛@ÊØ"ì>,@zªÁ	J,?Ïfކ]§¦?×Jë I÷p@	wß 'á?þZ2H|›‡?ê,n¾#¼ž?ѺÔýÐ
¿åøÙÀ¦"ê¿ê7ÀÌ
Š,¿é¾u†"Ú¿ÆÌÉ\Tê"UNASNone?À&8µW$M?ƟÿçÒó€?ëöqÒª6î?ƟÿçÒó€?Ö/W[$åÈ?Óäý_£ô?äèTRm?Óäý_£ô?Ê)èÈzåd?°ðØò³˜?éu…ÍáF§?°ðØò³˜?¨Ü¥ÂËö?˜4õ»Õ5Ï?îr5£Ó@ ?˜4õ»Õ5Ï4FGL J1752.3-3139?îË^ƒÐ4£À ]ˆ¿À9¡w·ÒjÀ;HóŽØu@DPó7š¡@õö&bjX?Îê—Ä'P?ÐY0ó½Ò^@uH#…@F?ðèҁӿìTS^¡Ëí?ïÜùjºˆý¿è–"ì"¿æ•BA˜ü'¿é7zàÆÔ»¿ÞR†à"d©UNASNone?Ù~ ¬D8¤?Î&'©}ü/?ã@¯©Ýã®?Î&'©}ü.?á-iOšs?ÖD0w!o8?Ý¥-`Ë?ÖD0w!o7?Ùü/~îç?·i»w^µ?ãuè@ˆŒ?·i»w^µ?±¶còlÚ?¡CÇQ¸¢y?íÉ=3²d?¡CÇQ¸¢y4FGL J1752.7-3040?Ùg#~qÝÞÀÅ«ÀãŠ~À9¶4EêPÀ;?ª9ú͑@؂Žs@–üõ‰"?Íi#šŽâ?âAº°j–@¥ò`L–?÷IŸsxGº?ï!FÁÛW)¿×Ï?"ª¤Ú¿ÞïåÿÏ®¿é¦2Ï`%¿ê€™'ódç¿ïö×B®\UNASNone?˜:}oÄ.¤?¶v…_¾q?ï>,ÞŠ?¶v…_¾q?Çf?Ö2ˆ?Ï ÿwȟ?ê&p
s]û?Ï ÿwȟ?¬ÉIjT?ši¼ð<΋?î3oßûiZ?ši¼ð<Ί?ˆœAk‡…?pÑKÈi¸?úQáÊ?pÑKÈi¸4FGL J1752.8-4449?ûÞávfÀ"¡ÿ´€¥­À:9·	ìèÌÀ;éBí»YÞ@—M;@3ÁÎl	?Ç·&'?Ù_™ãÁZÿ@çń/_@KÐÈ:?íÚò)}§Ì?ì,â·Ý!¿Ù( ú"¿ã	Áv,'¿ëÜ>"Ë¿ïû¬áxUNASNone?™ÕvYx¹?œ)·"\?ï1TM3":?œ)·"\?ÁYÕ
ÿòº?ÄÞæÎhµ?멊½@R?ÄÞæÎhµ?ºlå½|0b?­ËŠíÎô ?ì²cHPyô?­ËŠíÎô?Ã|³±Bª5?§cWÀ`þ?ë Ó¯Us?§cWÀ`þ4FGL J1753.8-2538¿é÷'H#Ð|?À?^¥&ë|À7´ªÄdHÀ:L$BÕg¦@þ¿e @ìÊì"?®c_/n
?Ô/ÆÂÃÖ@#š {5?øƤfý5?áÔS»d?Ù0W¶ :ž¿Ò•ŸäâBU¿â€Õ}uv¥¿ék¡~•\H¿ì¡¶hÝ9,UNASNone?@š{´¬á?GÐ¥WrÆç?ïûÙaþ"?GÐ¥WrÆæ?Z¸c•3£?f›"bPç?ïò£Î57æ?f›"bPç?°Û·Æ¹3ç?£á¤88´
?íä‰(ك?£á¤88´
>øRû"3üÍ>îÃ÷aã"s?ïÿÏZ÷˜>îÃ÷aã"s4FGL J1753.9+2443?î'Gœ{ì@7û¨'j©À:2@h¥ÛÇÀ<[š'Í¥:@҉¹ý'=@ÅΞ^$y?Á"K©¡¤€?¶@+"-t?õbØ<l˜@
ÒÐ]t$?í˜ø‰éù-¿ç$‰¿ß~Q€ž¡¿â7 €=¨¿áXK»À5¿ïÿ¬ÞoâfUNASNone?ïþk'ûû?(À/¤û°
?)M€@Gë…?(À/¤û°
?ïýÎôZìü?IíUŠ(à?1ˆ](˜)ã?IíUŠ(à?ïêµ0±J?qÊ|ŽN¡Ê?eJÏùN¶9?qÊ|ŽN¡Ê?ïù2,v{Ï?5›•Ÿ
?K7N&ÃN?5›•Ÿ4FGL J1754.1-4333¿ì'jÑÀ!ϪŠ'¥aÀ:åªô4ð£À<Taä ¦i@!®ˆ Ø?áÔ"°Õ?Ú衾V?èçԐ­?þHż7SS@ª¥¼'—ó?ïù
ãˆÐô¿è¤±ÅàI¿î½_œr½?Ë®¿Æ~ÿå?Á4Æ[C¿í¥qß@lØUNASNone?ïû¶é•O5?Eæǜò?A$YªÃ)‡?Eæǜý?ïýÒ#X'c?Qå«[W<"?1nå;tç}?Qå«[W<€?ïS"•1S–?':`†U¦¼?•YՍP?':`†U¦¾?ïý
sÏ?7õ;¼?7§—äaÆ?7õ;¼ò4FGL J1754.3-4443¿¬ÔìR
‰5À"ûR†µ'GÀ:x.åƙÀ;Ý Y§;@NµÖ\@Ðä¤Yæü?È;>"õó?×Wôž"}@‹š°@2+5㼨?ïý˜F³B¸¿àžÜd…¿áø#'¬?¿ç²ñYt¿ï='á>sÙ¿ÕyF<û3UNASNone2FGL J1753.8-4446?º÷¯XÈ ?½60Í_¹??ì¡
ü¦í?½60Í_¹@?Ы¤i'ô?Îm_ÒÚÈÞ?çª-Ëlx?Îm_ÒÚÈÞ?ÇAç¼õ{?²]恍ê©?ê;/†¢?²]恍ê©?ÇÞ«Ž:ï?¥MýÔ
òB?êUqE?¥MýÔ
òB4FGL J1754.3-2915?è~­|Þ?‹¿üÙ`sÞ.À:<Ñ®³ÝÀ;Ï!CF¦­@V'ýž%ð@•§Yu½?ֆm'dsÈ?ïâp"&ñ[@c§@KIª?ýž€ÌC:?í«j¿îþ@5û?çÕk׿o¿ê¥_Ù.…¿íÛÇ4ÝW¿éñ\~†ÝUNASNone?²÷ögø6°?¿\³¡.F÷?í¡3ù*?¿\³¡.F÷?ǸŽÿ—xf?Ñ8(0¾-?êÜ@!å?Ñ8(0¾-?ÏÄwXᢖ?´#–ø²k?èâ)ǗZ?´#–ø²k?rÈ\ö"þ?ku¼ §ZÕ?ïÛòoFº?ku¼ §ZÕ4FGL J1754.3-3236?îMK°zÕÀðƒB?@À:ðéÇ´À;}ƒvA¥½@þŽøœ@·†ªØ?Óý31…´
?çÜÄA
Š@~}ÖÅt@7§î&!?í Ɋ"-?ìT4ÀQn¿ä3¬Õ¶€Z¿îF—> Y¿íõ~†mÿïÉ$i¢UNASNone?¨ù"2•q?²+/Eb'?îpmÜÖ¨ï?²+/Eb?ÄGµzŽy?ÍPu½p.z?êî¡xÜb?ÍPu½p.y?¿'÷ü>û?¨¦Œ"w(Á?ì@x!?¨¦Œ"w(Á?'zeã,H`?m|ÔèùZ`?ï¶hsNÞ?m|ÔèùZ_4FGL J1754.6-2933?ìZ\át‡Àœ˜†À9<;¨LºÄÀ:ѕç]qË@ƒÅ[¿Cw@á';×F£?ÇFŠ¡Y,?Ý°å:¬Ï@¬$=Ìê)@Õú¿ïàk]¾L?ïÚ¶š[`y¿à4v)R	¿æÉúŠu9h¿ìÏÝ=]X¡¿ïÿC*!<UNASNone2FGL J1754.1-2930?¤B"ëÆDã?«6}™0–?î»Ö±C›²?«6}™0–?¼°çéi?Ç÷Å(_c?ìn	ãÒÝ?Ç÷Å(_b?´|<¿•æÙ?¤hÞ@ñ?ípxh
C%?¤hÞ@ñ?¸X•ð3d?¦Pyí¯( ?ìÿ´íAù"?¦Pyí¯( 4FGL J1754.8-3200?ï¼î.;zÀ
*s±éÀ:€aº/;À<AÎm¶¼À@zS¶xM@XÜ}Cø}?Ò	}!"Î~?ïö@líüÈ=@4¿ÆÔæ!?í+ž{ÝÇ¿Ô5edd¯?Úø¦¥×¿ß½Á+®Ús¿ïýÝ¡s²?î¢ÊšÃeEUNASNone?ϧŸ –(?ʈtfF?«?è<÷Úw?ʈtfF?«?×,/¹º+?֕(ø•b?äiè#p¢ê?֕(ø•b?ÂÑ(d'N¿?¬'87ìÀ?ëKµæö,P?¬'87ìÀ?ÄM5Œ{‰T?¶·gÒ~C?ê천á«?¶·gÒ~C4FGL J1755.3-3937?ïð#¯ÿ>À žý†¨üÀ:Y‰SÑ8lÀ;5^†ž@'êF/dG@bû…Fü>?ÚâLÒ?Þ]C½oÑ@
S½Ö.u@ÚÊö†?ÖªtÞ#aY¿Ð4à²\Þþ¿æ<˘fÙ¿æÎG P¿í9Ž—¿ïû
¢ò)UNASNone?ИŒ²‡F}?Ê7z«oÀæ?ç³¹¦¼\Ã?Ê7z«oÀæ?âR9À5?ÒÆr7frì?Úå[Œ•Õ?ÒÆr7frì?Õÿ8Á=få?·§pG.†?åcŸaL?·§pG.…?Õ7Z,¶å?³¯‹¦y?ådRÀi¤?³¯‹¦y4FGL J1755.5-3734¿Èi8~Ó¿kÀÂu%F
¦À:3qxéêÀ;´Ç%Ãß@àÃEJ7@¹}£~?Æda¾áҘ?´¥sl‰@0?ðËoÕzñ8@å½ïD¿í
Û¢R¦?ïâN>Qtg¿ëô…þ²"'¿ÙÕp_c'Ì¿àÍ]ìDaY¿å3TÁ"tŸUNASNone?ïuÿ
'xË?'M¨ÔÑ2?'@»æ›?'M¨ÔÑ2?ïÙÍ¡'–?"µ~ü`Œ?s/y¾µZ?"µ~ü`Œ?íT<¨ü"T?©Óûê<?µ^¸í`?©Óûê<?ï2AƑÿø?ˆ"/à2€o?™·Ç-À?ˆ"/à2€p4FGL J1755.6-2050¿ÑÞÜçÆ¡@'¹"ËÜãÀ9£B,Ë:&À:èî4%¡z@-=¹Ic@$ ]Øù+?Ã0ÞÖÏ/¿ŠSa?Ͻ‡?Ç×[†Žz?ý£øJÛ?îœÂþí±I¿á±—¢H"Ä¿ë7Rè`¸¿æd¿1ٖà¿ïÿþó…õ?ïÿùŸé"ÚUNASNone?îh¸¿Þ†1?­16XØ{?©ttœô?­16XØ{?íÍ·¾X?ÄìÔet8?±'GR
F?ÄìÔet8?ëCHå×?©ÉºeƒP?ÂóöÜkˆ¢?©ÉºeƒP?íµ¡Á½?¢C€±²%g?²Ró÷2?¢C€±²%g4FGL J1755.9-4009?셕²'PÀ^[ÕêÀ:'ci[ä,À;±£_9M@/ðÚs(—?üè˜`´v?ÛúgVPo?ä%+¾IÒ1@!='AŽ@@¡~O'7Ë¿ïÿñh?ïþ¦>½·¿ÝÇv¡œó@¿â¥ýàÀõ~¿îßô╋î¿ïÃÆ^‰UNASNone?èAs¹L0ÿ?Éfúï˜	?Îú1Ï<?Éfúï˜	?ìY½	4Óµ?ÆZ«tCˆ?½2¶YbW?ÆZ«tCˆ?â ìIaùK?º	hãÜf;?Û¾'m<
j?º	hãÜf<?çE§îUIË?·šòŒPf?Ñt°#Ulm?·šòŒPf4FGL J1755.9+0953¿Þsñ\@0Åè´k­À;\Þê¸À<·k;¸=@"6°î[¾?úA
a'Ï@ƒû¶Å$?ïEj7¬>¸@¡¥×•~?û´Ê­7Ü¿îÖ¾ˆfko¿ïÿë<ú\R?ïû!ô›?ïšT	lL¿Ýº7~œh+¿ïþ"?½…1UNASNone?ïÊ4ì±é3?zó"WO<?z剧f?zó"WO<?ëÇ¢~©}–?Ðò…íëf?ÀávZ	ª?Ðò…íëf?îå$ØÁ|¤?—ç˜Ù?¡­²sè5Ï?—ç˜Ù?èWiPLÅ5?ÐTÚ·³Óœ?΢Z¾Ìë'?ÐTÚ·³Óœ4FGL J1756.3+0236¿éP²8·°@*áŒâÑñÐÀ:#}At>–À;ž³ì+6å@‰Àë,ß@¥½"J¥@?Óm©PÆÂ?Õ
ßâ©-
?ðßXÀ‹v@ÒU%v\?ïïB¾¤Ø¿è=-rH¿ìRþtå…*¿äÏ/!}¿ëðžc,ö?·ºú½Jù£UNASNone?é˜'‡G?ÈV앤(?ɟ•·âá?ÈV앤(?ìðÞd6«ˆ?ÃÁlרaO?¸yÞJ£º?ÃÁlרaO?äX°/[ï¬?¹¡Dé?×NŸ¡H ©?¹¡Dé?ídR‡­O?£MyTˆ?´Ýk•‡é?£MyTˆ4FGL J1756.6-2352?é":Ñh?ÝÙÓÛߺ:À8"d鎤sÀ:/4q÷"!@ҝ{PƒP@
×^÷\?Ør³üœHK?Śx§0°ø@'Í|õôä@"\d"ä×?íQ`_¼(:¿í?½ÅGó¿Ì7¤/¿èpó‹(¿åôÑÞ¯xS¿ä@GƒLP;UNASNone?ÂÓÙZÓ
Z?Ƙ泫Ѷ?ëK	©K<ª?Ƙ泫ѵ?Ð0%4^Ä?эûÚti­?ççíeÿPž?эûÚti­?Ѣ楆Q?¾ût)Ç?ç.Œ­<þ×?¾ût)Ç?É!Z'#º?¶M֞˜à?é·¸)v7?¶M֞˜à4FGL J1757.1-1926¿ïê릶•@Ķ¦ڝÀ9±RÝóe¾À:þ»dÅ|v@9Xo­·ß@6¡|¼ê?Ñ"0?ÙÛ¡¦ÙH@Ž¨¿§J\@Ç²0¿;?ïñ1Ñ3cÛ¿åÏ®&ïX¿çÓû_‡O¿èÃ^¿ìr±˜"à¿ïÿï¤h)µUNASNone
?Ó8öܘ?Ê5H']L?æc"òx´?Ê5H']L?Ì©{×ð+ö?З—S~"Ú?èÕ¡
õ?З—S~"Ú?ÓðFŒ·f?µËò!?7I?æܹ¤xÍ?µËò!?7I?È»‰‰?¯¡"ÿÈ%?éÑ>¾]º?¯¡"ÿÈ%4FGL J1757.1-3554¿ï#æÕÃÊõÀˆ.D¶é6À:aÀ¥wnÀ<|Dôü—@º÷dP±@/¦¥ñ—?Ìr‰µJúû?á§ZS<=@áè¢ì(³@:ßý¥?ïþ¾°nÈ¿å$@ò8— ¿Þ`\̉°î¿ç¸A¥f׿﵂˜Ì@¿îñ›MοìUNASNone?ØÝNÆ×B?ÍÂÛ,SÖ?ã'Xœ"^ø?ÍÂÛ,SÖ?߂"CÀZ?ÓÄã›Ùi?à>î÷ÞÓ?ÓÄã›Ùi?Ä"¶Cü?±i'?êùz[o?±i'?ÛB—/S"p?´6«éÊz`?â^´hV6H?´6«éÊz`4FGL J1757.1-2848c?Ĝ§²ëëÀßOC427À9¸™9!ŠÀ;!-w1@
2AEÆ@ðÛâêE"?ɇø‡eºo?Ò¡ÿěÐÖ@	Gcä«æ£@«.4ä³?ïã²,¿Üáàš´÷™¿äµü¦¯,¿ç´<G®ë:¿î2BÝË!Ò¿ïÕ ÞœØéUNASNone(?Ã>b"€ð?Ám¦9³›?ë0gw_ø"?Ám¦9³œ?ᤡÿ'D?ÓC=¤—½(?ܶ¼ÛÙx?ÓC=¤—½(?Ð8§Þq?´ù¸ÌE1?ç㬸pH?´ù¸ÌE1?Ó@Ä
X[Ë?­ƒ _ÿ?æ_ùSÒ?­ƒ _ÿ4FGL J1757.4-3125?à­÷"Rõ'À«ºÅcLÀ9xäû—»sÀ;‹w·Òj@²:öËú@›´áô|>?ÀÁ_Eà´á?ÕàèãƒÈw@ߒޔum@_5¤ ?ïš½ÐZ¡¿ŽWÚÌ-¯U¿â«)yv
£¿æª)¿l ¿îà÷Ií¿ïòè ¹UNASNone3FGL J1757.8-3126?tJF
á?'=þ0,Œ)?ïŠ.ÖçŸÈ?'=þ0,Œ)?ħ¼œ'?ËòÿðD¸?ëÖؘö?ËòÿðD¹?°&áƒCƒ…?¡Ìª¸µ?íû#ϗ?¡Ìª¸µ?³(¡<Ý?•n62æG?íšëØp¤?•n62æG4FGL J1757.6-2731¿ê¶I-v#?¿øÐÒëʾÖÀ:	 »aj~À:úÑ9C­@†"'&3@mâÀT?ÝlRƒÛlM?àëEþçÒ@
x¡UO¾?ÿm>ô‡|?ïó$Oj¡_¿¼‡!F÷‹<¿ÝA"Šfð¿ã¾¹ä¾¿ìÆÝ»²s¿ïïë€:ÕUNASNone	?¯~¹õAh?¹b›˜£Ü™?îô`«é?¹b›˜£Ü™?á"س2?ÔR‹p³"ò?Ü÷ÿîN™›?ÔR‹p³"ò?Ð?Ó1W?³«;èÈu¯?çö`gTw?³«;èÈu¯?Îïw©)¥?²â7¯È¿?èD:ⵘ?²â7¯È¿4FGL J1757.7-6032?ïý¼ã/à'À1/ס<%JÀ:4Ú§€âéÀ<iË@ے@œÝ‰š?ú
¦ç_ö
?ÆÍÆó?Û]õ¿	j¸@³·õfI?÷Ïxw
#?ï×táSl¿âYbqå ¿Ó™û꽿͝CÝ¥b%¿ì}y¼"€¿ïÿßéà
UNASNone3FGL J1757.7-6030?Ñ>*jð˜?Ñ75õ¬´æ?ç`êʇš2?Ñ75õ¬´æ?¤[}'*`?¹½åÔ|?îºH-^?¹½åÔ|?Ëڀ¡P¢ð?¶¥¸å?é	_׫×D?¶¥¸å?¨6	1ýÜd?™\'ván?î|Ÿlà"9?™\'ván4FGL J1758.0-2953?ë HªF$À0ÄÃéÏÀ:uK8¶ÈÀ<Tlô!-@-¡"¹ï@ÞZCBtð?Ò¥î[è´	?ïçùÿ4þå@U ÃÄæ?ýYnîöt¿îë\‡Ê?ï8tP3ôú?èëÏO^¿ã ž9%¿ï1…ý¿ïþ·á-VûUNASNone?'šÅ&À¬?""ïg*g¡?ïk)Öˁû?""ïg*g¡?³:zÄbÍü?î'ï@~?혰§s¦A?î'ï@~?»9uŠËD?¥‡ÒR…}Å?ì˜Ñ_.¦˜?¥‡ÒR…}Ä?zŧu"õ?o6¬€s-9?ïÊt±éº?o6¬€s-84FGL J1758.5-3219?îÂÞ_ù'Àv–€àe0À:|r®sErÀ<
ÿ"Év@{Ý/E'Ü@
õ ¨ìô?ÕA[j	?îL%þpÛ@hò'hûl@Ñð~Ø£?ïÌù"@F¿àÓm›
à¿ÒjwØ~±·¿êìgpQ¢¿ïãh¬'Ä?íρ'¼±UNASNone	?Ðö~êü{?ÍRé_Zî?ç"ÀøŠÃ?ÍRé_Zî?ß=A4
‹ç?×#!+p{?àa_eúº?×#!+p{?ÏnJÀëø…?·¿šÐIu?è$mOÅß?·¿šÐIu?ÉXVRh?¸SaÕ?é]?é©ê{«ze?¸SaÕ?é]4FGL J1758.7-4109?Ýԛ
©ÕÀ õìløÀ9w)@k*À;´è·äÞ<@´ËLD&K@³|™®'?´ËÞæ)ë?ÄxÑ¢õbî@
Õ¥á¦x¥@–'(6*?Œa¢²¿Ô±d ·¿ä€¿B Ž€¿àø>•'ø¿ê«ïxÉ?¿ïòÔÔK4UNASNone3FGL J1758.8-4108?Ú+™¾jß?ÊÀ•ü±?âê3 ʹ?ÊÀ•ü±?Σ4{¢?Ê>Ց(*€?èW2û¡9?Ê>Ց(*?áʂx@€Á?¸Ú]l¨Ü?Üjû~þ?¸Ú]l¨Û?Ý`£Y(†?°xí³­Û%?áO®Sk¼Á?°xí³­Û%4FGL J1758.8-2326?ïø1qˆ´ñ?ÐÏÝMx"À9B£©½ÔÀ:"Õ¿º•"@ "»tৠ@Ö«ÃgÉ=?̕͜«qÞ?ÛG>©@åídòÈà?ûºouá\¿Üçòº•=¿ì½FA­?«ƒ¾ÆÎu¿á'§àÚ¿é¡!ƒ†Ý¿ïÿúÁҝÇUNASNone?Ç')Ýn­T?DZôȕÉð?ê65ˆ¤T«?DZôȕÉð?´šRÏØÑ>?Åbklbë?ílµ¦åØ?Åbklbë?ÎAÕ7@"t?´_9?èoŠ²/Úã?´_9?²§;
±_O?¢ÃšMïœ?í«ž©Ô?¢ÃšMïœ4FGL J1759.0-0107?绘gëÝ£@&7ÏÃøõÀ9Û÷÷oÀ;c§¹íÍ@ó!6Ü`@ƒÂ‡çÀ?ÍÃք´?Äï@£3?òãII.?þ\ÀJ]qJ¿³G'±Ê½Ô¿æ‹¨ñf¿ë··¶ùҿ絟=Ø©¿ïÿòɶ—×?î*éŸ¡UNASNone?îׄüš?©ˆúS™d?¢‡°>n6d?©ˆúS™d?ë3oŒƒî?Ë&Ø¿_d?Ã3ŽAÍðI?Ë&Ø¿_e?é¸z
@/?²õb\ùàÌ?ÉÖÿ¿D?²õb\ùàÌ?ìŠð8i
ª?¨ôÉ«é}?»¨~<·ª¶?¨ôÉ«é}4FGL J1759.2-0243?è¨~Sé1@$¢hn~bÜÀ:cÒuðGÀ;ì†<Ń,@f°@O%'@Ó€™?Õól^MW?ïTów[0@ÀŸÀ$GÞ?ÿ=±nwí?îU€šÅÄ¿â;`"¾ŽF¿ãÝï3ÿáÍ¿ïH­M«"¿ïÿXJ?ïý÷ý}ÚUNASNone?Ý4:žZ¶?еªµ?áeâ°Òþ¦?еªµ?ÉÆr·;ø?Ñ˗‰ÿÑW?éŽc}1?Ñ˗‰ÿÑW?ÑTÆ(\V?²á@jò©?çUœþëÑÕ?²á@jòª?žqËÄÛù?"4¼="ó?ïÌq¡Ù!?"4¼="ó4FGL J1759.6-1850¿ãÊnüc"@îÒ£¦bÖÀ9'ÿ#a.À:ãóbb˧@•o¨@Ö¥†6æF?Õ/š¢X/?áþ¡ñ@XÈh¹ý½@{èP¶Ñ¹¿é¶V˜í!?ïûáÝÖ	Œ¿æ!['—¿é¶ˆRIxð¿éÀ¤ ^¿®<kb›øçUNASNone?ÕþH]A¾u?Ò`]v·*ž?åÛÑ_ Ç?Ò`]v·*ž?²Z#èCww?½WµŠ{ìq?í´»'÷'?½WµŠ{ìq?Î91Á=(N?´þ%U"Ö?èq³°µì?´þ%U"Ö?¸!Ótº\Ç?«KäJš?ìûőh´g?«KäJš4FGL J1759.7-2354?î1™äÏ¿Åe¬­À8b¥)œ±À9™‡(}͋@ Ÿ:o°­@€ýÁ?ÎAN)Ø¢?΃*Ar>@€¦ƒŒçÚ?ûÞ?Þ½:3¿èÑÿ'›?çk<Žü‡¥¿Ö<×ÁóT÷¿áŽþµýþ¿êȸÀü4¿é–ƒ?4{UNASNone?¨åqÅAÙ?¾ÆtGã±?îvñ¨ã«ã?¾ÆtGã²?ŒˆºD(õ ?æUeçoö?ïÝï\+?æUeçoö?·oÔåš?£góÜ?ípãM?£góÜ?…Eá«Þºv?™íÝ?ïªèyP…?™íÝ4FGL J1759.8-1250¿ï¹îyœ@5Ïò=À9¸Ÿb0wÀ;A;ʸ@ýz¤6@ÝâïN?ÉÌ7;*£m?̱8òÔõ@ùæ
‹t?õ©%Lj½?ïöBçÜÌ¿çÖòU'¿ãêÕ+@«¿Þ]¨[ý¿ìÓ~AÏX¿ïÿð懈öUNASNone?å¦ÆAÇÛS?É˝F+â¤?Ô²s|pIY?É˝F+â¤?Û^õYd<!?Ó^òMŽÇ?âP…SMáð?Ó^òMŽÇ?âAœ䔬?¸G²Š8¨ú?Û|ÇÜ6Öª?¸G²Š8¨ù?Ëåü,ӗ ?­yÌ!Ç?é€ôË?­yÌ!Ç4FGL J1800.1-0323?Ø£m
ž2@#•¯)M×#À9r•Q5}À;3Íw·Ò@Še¹ä@A#ßYw?Å¡«¡Y¢?Æ»Jî:Ü@8'¹ÑG†?özՖ´¿ï˜Ô!Õ½·?ëJþ€ù势è–ý»'"¿æªÑù\¿êLŠÝ"T¿ïÿö$´ë/UNASNone?ä%5µäÆÓ?Ð:(2y6p?×µ""6rZ?Ð:(2y6p?ۓݞUÓ?Ôh‹ºz?â60Õw?Ôh‹ºz?â =¤†L?¼½ÝŸC?Ú¿"·âóf?¼½ÝŸC?Ñ:	L4S\?¶ÕÏ| ?çbûYåÖR?¶ÕÏ| 4FGL J1800.2-2952?æ´ýâÿZÀ	³åZbL%À:<†&öÀ;Ðכ\è8@ü±A%@Vî#^©Ú?Ò2B…Þ?éC´öl@©Ì1œZ>?ü°Rÿ?³«`Á`Ýæ?îtOȕ/¨¿áƒŠc›±¿ê0ô)2(q¿ìÀØ7d\¿Ý@*<•UNASNone3FGL J1800.0-2955?=òËãÃ?Š|ú]¢]Ø?ï»4Ðpô?Š|ú]¢]×?ˑâºÛ¬Ë?Ѐ½W"û?é‡QIÍ?Ѐ½W"ü?³îGïf—?£½"úÚA*?í'73-?£½"úÚA*?'ÿ@¹u?u¦Aó¨DC?ïpûR4?u¦Aó¨DC4FGL J1800.2-2403c?í""æ
I=¿Õ¾¤žvÀ9:G#«À:A>Ž±@"¾]ž@zÑî0Ë?Ð輁ûî#?¤8ût*b?çk;³´M?ü@°?è‡G½-óX?ëÍGF®Ê¿éö;ÏÆ|¿äûñþ_–é¿ãMÁÔÌ ¿ágÑ­ÝUNASNone1FGL J1800.5-2359c0?ښ¸ü:úZ?Ò\›»Eõy?â²£â'Ó?Ò\›»Eõx?à¢äŸÀx?Ù!('Ÿ™«?Þº6À~á?Ù!('Ÿ™«?ã(§…ñ?¾mìÎ9bˆ?Ù®±ÚôÒ?¾mìÎ9bˆ?؆6¹1¨?ƒ{#?i.?ãõ<ä£g-?ƒ{#?i.4FGL J1800.3-5237?Ô6ò¡åÀ,!ámmÁ¤À:óp–kðÀ<jm³aÁ¼@õ^£ylS?ó²õú:Ä?ÚsW%*ÜÍ?çZ)ûÒ@p¨ß‡ºt?ýÒv发X?ï«P°ò{³¿ìi¹Âƒó•¿"z±ÄU&o¿Ý#½¿"©@¿èW B•¦Æ¿ïÿ¬óéqHUNASNone?ïÜЭÅl?tÍfq°áÃ?q—©wÊP?tÍfq°áÂ?ï eˆ.ã?¦(°"¢Ñ?‡úæôG"?¦(°"¢Ñ?î^®x-Ë?œè'q#CX?ª•}#H?œè'q#CX?íÛ8"h_ã?¡­÷ÏöZ?±&;ܽã?¡­÷ÏöZ4FGL J1800.5-2910?¿‰òØmÃÀ`¾¼hÑ{À9"ùdŒÀ;æA@9
6u@¨âù3?бuBø";?Ԕ@~Ë7 @]›¡±–?û÷Zþÿ$?àɀ2Wk?ìùŽâ0Œ:¿áÑ>vˆH¿ëGÁ	Ë¿ßÛÄhû¿ïþ)›Ú¼zUNASNone?ÏÛ´•V?ÉâI¿³W?è	Ú¼?+?ÉâI¿³W?ÜIŠ7Dp?Ôs[ƒ‡ó]?áÛ:ä]Çó?Ôs[ƒ‡ó^?٭ό"=d?¹]*A}´u?ã)9µáN?¹]*A}´v?´'±±ÐJ?§evjú ?íl[	ÉÅø?§evjú4FGL J1800.9-2407?íeȏèâ¿à]Ÿ¤u–À8DAYA»À9Îb뇢÷@ ì1"‡c·@Ĩm'K?ÂÓÝ7S(q?ÂÏڞF§"@
 ðbÔ
¯?úo·UlC?ïÿ&@±v¿ì§w¨®	"¿×
;&òˆ¿á¯`«;'¿æóû_‡O¿í¨]»WUNASNone?Ò}ncççK?ÏFĨph?æÁHÎZ?ÏFĨph?³5ÛT]Rš?Ã@m¡²Ó?í™D•tU¬?Ã@m¡²Ó?×r;ȦË?½QŸ‡DT?äuÆ⬛?½QŸ‡DT?š®¨™Á4?®µ%!Úó?ï/ꊻ1ö?®µ%!Úó4FGL J1801.0-2802¿é"	ŽJÀº;<ìðYÀ:+PâÌÀ;¹ë1;â.@÷§kê4@Ôef—?Ìô¡}Ð<?ãÍ?ïXz@¢G²?ÿÝ#?_¿ÀçÉ'{Äò?﷙ÊAR¿Ýö5{âÏn¿ç5šìð¿ïâ&›u;ì?ê¯òkÂƺUNASNone?€á쵨?–?¡©‹ ù?ï¼xM)_?¡©‹ ù?ÏÇYa(¸?ћ$nÓ-t?è)§¸5Ó?ћ$nÓ-t?¦§¦±¯?""
zq?Ÿå?""
zn?²	JB-ÝT?œçދV?í¾Ö·ºDU?œçދT4FGL J1801.1-2626¿çE+øœïñ¿û,0ªÂ¶ÉÀ:X`£®ÆRÀ<5ßüTz@ k\sÉPk@DR´Øº?ÒիÒ¼[?ïكÿÔa@þB҄?þ\×w¬	?îŠ<d4\ÿ?ÓÔ
c†7<?¶ûlâU°¿À]6fïMU¿ï€¤ ]Øù¿ïö-ƒÆÉ~UNASNone?~,7xY?‰b/›D×?ïçßN?‰b/›DÖ? à«¡Œƒ?´@IFQ#?îñõEç7Ð?´@IFQ#?Á¼#ØzÓ¸?µ=ü(˜ýJ?ë÷	áK?µ=ü(˜ýJ?b,LILV…?V¯ábåi.?ïíÓ³¶³ª?V¯ábåi.4FGL J1801.4-4307¿ëµ!dzÀ#³y1DEªÀ:Tb(êÀ;ÛüwµCC@½±$¥¦Ã@œ˜D/ú?Ò§›ûH¶'?ÖáUðÍ]@UÆ2o?ýL…>õ?ïÿÕm…>™¿Û½?¼¥!¿å¤œâ¤O€¿èGGÝdI¬¿ïÿþÐñ?ïõv'[¸UNASNone?ï˜\"2$?'Hõf{U-?‰èÚøów)?'Hõf{U-?ëõÿÃi8É?Å8V‹ã#v?À(ò[Ü?Å8V‹ã#v?åÄv_N"?³ÅÁBá±?ÔàwAbÚ?³ÅÁBá±?邘Ô6Ã?³Ó	oŸŒ>?Éõœ¯Ç$ó?³Ó	oŸŒ>4FGL J1801.6-2326?î´á¿Ô,™î˜ÏÀ6À.¬»µMÀ8óq}ñg@bQ#35â@IN…Ÿ?ºÍHÁºË?ÔiQÓ1jÜ@",pCß?ûøúJ3ß?¹Ëw7Dù¿çõYé€aº¿Ùk	ä/iû¿è\ƒ3&¿ê˜È]ý6L¿ïý ½é¨UNASNone0FGL J1801.6-2327?ÓI¤m'î²?Ù[‡ñöF?æ[-É6ˆ§?Ù[‡ñöF?c'ú#á)?tv™¬vc?ïìØ~Ü?tv™¬vd?´'kšaŸ?°p]A·®=?ío²œì³Í?°p]A·®=>ß'IfØöF>Ü%ÔŸ¨Ù?ïÿðl[L">Ü%ÔŸ¨Ù4FGL J1801.8-2358?ï€ä•uú¿ãŠoŊ¹,À8''Œ6À9îC–Wź@!Í-Ŷ@e¦$ÂW(?¼"T=ïÐ?¢¨süüë?ñä¶Î]Ç@W``u?Áüža)?ê¶( Þ†¿äµešŽŒ¿åAÍÊùö¿ç™§ÜR{οݡ…Æ}þUNASNone?Ò©˜í"?Ñl
ÒÝ ™?æ«83‰5þ?Ñl
ÒÝ ™?Ú:îÂ#?×â汌$h?ââˆó·žï?×â汌$h?ÜÂQÔÐ-3?Å9‰å‰n?áž×—éf?Å9‰å‰m?Ú¤Þ+ڎI?Äò›ûi"Ô?⭐ê¸Û?Äò›ûi"Õ4FGL J1802.1-2652¿ì3¼'åqÀÛšþôgÀ9Ë
By!TÀ;U
×ÊVÑ@ù
ö¸®ˆ@c4ÅÚjD?Ì/ú;É°?ãA³ß@ñ@ûÍxÄ6ü?ö"Gx¯p?í¡ƒræ§i?ï5+ÆWgÆ¿Ü2+`ÖÚm¿éNÜd…¿í/êß‹4¿ïÿa>ß8àUNASNone?qä½ÆQfÓ?|­ Xõ?ïÜ6"s]2?|­ Xõ?°6u‰3è?À,Ƭbï~?íù1Nقþ?À,Ƭbï~?¢mV' a=?'ÅQˆDp?îÙ*–Õùí?'ÅQˆDo?N¸†QãÙ?<£€Ö ²Æ?ïø\Þk‡?<£€Ö ²Æ4FGL J1802.4+3634?ïé_‡½G@9
TûÚ×RÀ;®ÉÀ¨ÒÀ=L-·É/‰@<# –x}@©Ã}˜²?Ô¶Òd'O?ëÄ=aŠ^"@£ñb®K@k
>pN¿ï Å®?ïýáý¶y¤¿×6ÿ[x³¿æ`¾ø¿ë)ZÖ¯O¿ïÿô!O…úUNASNone?Ñ|øtS?ÐÙ²¨Ó?çAƒÅûÖr?ÐÙ²¨Ó?Ͼʽ‡›?Ò4š/‰‡?èMPž;?Ò4š/‰‡?ÒpýÀ6ƒ?¼KÙÿ?z?æǁrä½?¼KÙÿ?z?¼13Bú°?¢m/xÞ=¦?ìyٗ¾ª?¢m/xÞ=¦4FGL J1802.4-3041?îQurƒ.À+"¼ÃjMÀ9¢{oâæëÀ;ÍÑÑ‹è@dÓr®HR?üېIŽ¿K?À¡u´6S?Ö
´ôhó	@åB˜I@†â8™Ït?ﯦ¶¸ŽQ¿åé,êCÖ¿Öl^"9¬¿Óoô¤Ø$¿åÚpú>¿ë©ØÁw¯UNASNone3FGL J1802.4-3043?ÓÁגP?ēœå|ÐK?æ6ÿ×õ?ēœå|ÐJ?Íï~Úa?ÑvCu¶?è" Ig¸¾?ÑvCu¶?Þ×=
\—?¹i3ë/áŸ?à"ay~Ñ´?¹i3ë/áŸ?ц_åRÇV?²ð y:œ?ç<Ð
VœU?²ð y:œ4FGL J1803.1-2724¿ïÄ5aWŸŠÀw_}>@À9m@wÏDÀ;÷¹à`þ@4úXKE¤@·Í+d2?Äé‡B©ó¯?ÐTÚ¢ÎL@Jd`Ò©@\+ž>nü?ßeˆÜ?Çõlh³ó¿ç'•`$¿çÁý &¼¿ã.ÕÖ`ÊE¿ïÿöàœjUNASNone3FGL J1803.1-2728?Ìy:Õ?Ä=N¿©ˆ;?èá¾{þ±K?Ä=N¿©ˆ;?àÁÄñ8k…?Ô0Wã¬|?Þ|v(ø?Ô0Wã¬|?ؗhŒ4X?¸óÝÇP?ã´s˹åÔ?¸óÝÇP?Ô3¼OX¹?¶3~Bÿ?åæ!ØSö¤?¶3~Bÿ4FGL J1803.1-6708?ïÉsøq	À4[çÈіÀ:èÅPØÀ<Rdë<#@ü:à>Å?þ߸Í;‡–?º†ÕFÃÞ½?Ð,âxY@|¶"‹ë[@à[8Šàï¿æË£¢1пۮ!æڕ¿ÝW˝>?¿à./ˆƒÇ ¿êÜV|E¿ïÿÿ&¦³UNASNone3FGL J1803.3-6706?çÿ¿¶XD?Ƴ§'_ˆ?Ѐ"OÓx?Ƴ§'_ˆ?ä'+¥£™¦?Ö¨»DËûU?Öû¨´¸Ìµ?Ö¨»DËûU?Ñ1™™ºb×?³S…6@(?çg33"Γ?³S…6@)?ë]ç·b?©ÞõfJãP?ˆc÷Á"y?©ÞõfJãP4FGL J1803.3+2425?ïHi"Ym¾@4ðx…LÛ{À:SºÜ	€²À<
A¢a¿@#úVå@¾"[Có?Òñý=­àx?ä㼝ª R@™Ê&)_u@¢+'ôØ¿àí0_nO"¿æߝ‰é"¿ìùXç!â©¿äŒpPÊó¯¿ï½þž0§¿ïéÜ»WUNASNone?ã» Ú1¤?ζH"àAÎ?؈¾KÆ¶?ζH"àAÎ?Ù¹ 5TWÇ?Ô×BGI?ã#/åUÔ?Ô×BGI?ä7|'Cƒ5?µcRúMŒn?בûxù—?µcRúMŒo?×JÒ¶"?»"¶Ñlˆ?äZ÷}–¤½?»"¶Ñlˆ4FGL J1803.5-1639?ïÇ_>Ÿ°@,ئãÀ:"¿Z'ÈÀ;ß[.ú¿N@zƒEÅ1"?þ­<^Uí?ÙÓ»¾Ýuç?ïBR‡"Ä@¥b?8È?õ£Þ&;~?ïí(Œç°¿ç|˜×ÒºM¿à±Èà5j¿î'á@øÔ¿ïÿÅGMƒ?íaâ"oUNASNone	?ë	¼ës?Ép{våX?ÃÛ¹Sú5?Ép{våX?×¥­1úc?ØZ÷Çom?ä{­)gÏ?ØZ÷Çom?ק†%¼É?´Íbؽ… ?ä,<í!ð?´Íbؽ…!?«'ðÑîý?¤˜ðµ'õ?îGÐòï¡?¤˜ðµ'õ4FGL J1803.7-3207?ÞÍ[NˆdÀâP.ì|•À:
5Ä+mÀ;ó`µL~@ŠŸþ…,@ù×Vé?ÌÍ£6{g?Üp¼`mþá@;=ïí™@ó
Ýԇ¿°žaÕ]-?—B&rþ¿æÛÆ/#Ùú¿åÚv»œ#¿ïü`Ÿ±?ïÖ¢
±nUNASNone?ӓ–Ëy'?Èy]zwc?æ64šC}í?Èy]zwc?åŠf'‰ˆT?Ó%¾oo?Ôë2ÚìïX?Ó%¾oo?ÐÅǔÅWð?¹sþ윌F?ç5T?¹sþ윌F?å¾;Òópò?¹	Ñ«\?ԃˆZ?¹	Ñ«\4FGL J1803.8-2908¿Ðm…ò¸ìXÀ[
Ø/×^À9··ä|À;UûKeY @X4Pi¥@(©6Ŏë?ÏLáÚûä'?íÕ€ÙÚ@Uí¡Xª¼@¢ŸÒ™?çˆ]‡º¿Á":šZ´¬¿èœRnM¿ìz¨<ʋª¿ïÿ¹ô'ô<¿ÞՋ¸/‡UNASNone?œòîöj$?¤>+ ðC'?ïhˆL®ß?¤>+ ðC'?´ï×ì£Û?Âp}i5L,?íbk"ž?Âp}i5L,?Í}PÂсž?µìdo™©8?è «ÏKŸ™?µìdo™©8?Z%GV®W¬?CYäN;r"?ïòí\T¨Õ?CYäN;r"4FGL J1804.0-1124?­r/b0œ@r€Æ^À:)vþUÀ;ÇáR•Ï
@D•pÀ–@Ê)"]È2?Ñޘ\Þ|?èd÷eýŠÛ@•—'$@8 GÉa?ï69bwCƒ¿Þv¦…:g¿å
¾"Š"¿îp;Ñg¿ð?ïÿþˆ0»ŠUNASNone?æhì÷Hr?ÏñÜTB?Ó/Î&o?ÏñÜTC?ÐD¡)ƒ:õ?ÑÉoƒÎ½?çݯk>b†?ÑÉoƒÎ½?ÔMŽ¥´r?¶(ºÍÈÄ?åÙ8À-%Ç?¶(ºÍÈÅ?ËÝå÷ˆö?·;U…¤o?é†';Ã?·;U…¤o4FGL J1804.4-0852?æú_]GÚX@ò[1~þ
À8ùg+ˆDÀ;	q(aH@~öº†ú@¼R?¼©HðÕ?ÁØQeMa³@›ð™Z¯y?ÿªñ=D"¿×
P`½§¿ápv̗¿èÆ6°–5¿à½!=èBõ¿éþ=½Ð°‡¿ïýtÀc‰UNASNone3FGL J1804.5-0850?ßÁ£VþÒX?ˁw¬­L?à.T€–Ô?ˁw¬­L?Öÿŝ]%?Ò;aXÕt ?ä€w1Qn?Ò;aXÕt ?ãÿöûØ¢ß?µ60û4?ØNºB?µ60û4?؅…"iӔ?´·xG}_?ã½=5Ë5?´·xG}_4FGL J1804.9-1745?èâÎ"ûñ?ýjJ÷uÀ8ñOýnUHÀ:¥}§Ë‹"@© u@t@ë:Æ¥k_?Æׄ¶³…Ô?È#ë†Lá@›´&Ú@š€©•?è°×£Àd	¿Üúû´@å¿è·—{ž¿æÀҝòâ¿ïátYn0_¿ïʓ׸¹UNASNone?¼5ñŽ–?½/ªñÓ?ìyAÜß.-?½/ªñÓ?Ô+f­d¢B?Ñé¤èuöð?åêL©M®ß?Ñé¤èuöð?×ÝÌΉ–s?¶ónœñ2ü?䘻4Ç?¶ónœñ2ü?Ñóh»_Y?°¦žØîx"?çKô"PT?°¦žØîx"4FGL J1804.9-3001?Øk.Ƥ3uÀ½–ÁxôÀ:NBM'iÒÀ;Äq£±J@š&\`(@
r¡Þ¹?ÒËáÀNå?é¡Xª¼Í@XØ>?õ5ßðëåí?éŸåŽ?Š*©_Ù¿â©}g^ß¿ëY‡ZÒ´m¿ïíVy-?ìÐý³õeUNASNone	?"FÒªÎû‰?¢±¯鍊?ï]Éj©ˆ#?¢±¯鍊?Ôl^RÛ?Õ$¯ñݺ?åÉÐõV'q?Õ$¯ñݺ?µS´<ÙÃ?¢àÏf¸è?íUŸéxdÈ?¢àÏf¸ç?zÓ.I-Y·?kñrt8†?ïÊY£m¥L?kñrt8‡4FGL J1805.1-3618¿é;ËfëcWÀóÜìՁÀ:wè]À<Rµðè5@VðqB8?üç,å;Xœ?Äôe˜
Ma?çuÜ%/dr@Ÿñ=Å]m?ù·Ÿ•g¿ïøI©ƒò?ïÿߞ¶Žó¿¾í¼[t'¿ã؃ÿÿT4¿ïÿþR€ÖT¿ÞÛ^ºËmUNASNone?¡HøXj'ˆ?¸ÓV^?îëpzyVç?¸ÓV^?");¯ö—˜?£_Un$6t?ï^¶"€KD?£_Un$6t?°	¼šÚ?¡-'à~ÃÊ?íü^Þèl¥?¡-'à~ÃÈ?p}éOלL?Xþ›Çn%?ïß-`PÇ?Xþ›Çn%4FGL J1805.7+3401¿ç69±28Ã@7ª>iƒQÀ:A8æÑZÑÀ<?¨Ï—'h@p4Æ[D@…6…Î
º?¿m´¹Zª?Ó\K$Á€h@ûd8Š‹@óΆ‹Iö¿Ó˜dMk¿Óɏ*ªÎu¿ç
´¾¹
Ó¿è¬.È—‰¿ïüVB+ô{¿ïÿX°›>UNASNone3FGL J1805.9+3407?ËÁ¯–"û?ğÐuXU?éºTwB?ğÐuXV?Ö!èfF…?ÑC°ôæ?äïÌüܼ?ÑC°ôæ?ÒZ®?uÿ[?·V¸+Þa\?æÒ¨àER?·V¸+Þa[?Üã,-¤?³ŽžZO?áŽié|r®?³ŽžZP4FGL J1806.1-3344?ïÕ
_'™:ÀÌ$·omÀ:KX+:@nÀ;©$7í­@*RÁ@|¦CÌ?Ë÷Ám9Í?ºÛ~K››?ôC‰!|QŠ?ü
zW_?ïè³}pn'¿¶1NA+™a¿ê-uïpeÄ¿Üú"[ADC¿ç©E©W|¿¿çh̽]nUNASNone?ïϤªñç?|܃]ÄX?x-¸*‡-?|܃]ÄY?N(k†?µSêS¾?¤uyG¥?µSêS¾?í'`ï½Á?¨ð(cƒ?³lø'Qú?¨ð(c?ëhÀœf?§"h3Ø?Ãê\üé²h?§"h3Ø4FGL J1806.2-1347¿ïV'Iq@ͨ_/:€À9d
`:Ó;À:¦R©@@P€u[KÖ@<ÿ?æ"&À´½?Ú|ûî"ˆ@Ô²ÄãÊ?@Jîí^Ù?Ý·äx:#¿Ì"è^x±¿ëêQBóH¿éªÞe{…¿éipafø2¿ïãý5Jd¨UNASNone?Ðɦ*­?ц±®èzh?ç›,êñ)u?ц±®èzh?Æt]ù`ém?ËWpëåw?êb聧Ŧ?ËWpëåw?ÙYÈÞÂ?¹`†¡N/!?ãSx›žö?¹`†¡N/!?¼Å'Þ{‡?µȅ2ƒv?ìgO½0?µȅ2ƒw4FGL J1806.2-2126¿ê†–?(†¬¿Ð)TÂÏóÉÀ7œ;
˜	wÀ9{ÛàfÅ@øùSéa-@¯R¹
x)?¹nV\ƒ?ÔfÏ­QÝB@œýÒ(V@‹Ù_'F—¿ëÀ³ï†59?äɂ—½¿çEfîVŠ¿æ;_ýk¦¿îCC¡•f"¿êÕ!Ð4`ZUNASNone?yöô•Í—¹?²fwt}?ïÌÔdÑ?²fwt}?yãÉÛÕd8?‰GÍTäf?ïÌ8lHU7?‰GÍTäf?¨k-²ÎèE?¡.ì'I?îyM$Ó{?¡.ì'IŒ?O°ù"ù–?Cæ—Vh¾S?ïøÁžÁ ?Cæ—Vh¾S4FGL J1806.9-2824¿î3,¤EÀQ1eәpÀ9×]	ÆR_À;i²lÏ64@ãÂh@>±Ä2ÊX?ɺwàŒGL?Æ"³‰.èK?ÿ9MÿgSÌ?þÒ&"©x4?ïøò?Mé¿â›`
†Ñ@¿éÖJêà¿æá@øÔ2¿æp,XN¿äiUßZ˜þUNASNone?í´%}}aˆ?±Ë7±"Xé?²^Ôó¼?±Ë7±"Xé?ë\Ù ˆã¾?ɍí"«?Œ›}Üq	?ɍí"«?é´+ì«T?³¼{Žó˜¶?É/PMR­¾?³¼{Žó˜¶?åõ3v	3¹?²^$'>?Ô™혋?²^$'=4FGL J1808.1-1234¿Ým4<@
7S½vÀ9—žþ]h'À; Y}I׺@9 M'Úä@A*¢jùs?Ëub'¬K?à™Ã‹«@çԝ{¦j@Xbz¥c¿ãæ5‰NÈ»¿ÕÉ^BÖiY¿å¸ßDž•'¿é"+Þ«¢¿ïwj·-ÿ¿ïÍî'Ò-UNASNone	?‡ÙûE€'?†#Շ'Õ'?éÿå?†#Շ'Õ'?¢#î.®Œž?®L'!\ô?îÝÁ6?®L'!\ô?²oŸUT(? >ÌE傂?í²Uzý? >ÌE傀?°C-ÄÊš?•–¼aA'?í÷šGf¿?•–¼aA4FGL J1808.2-2028e¿ì¯Ðɱ'£¿ÇN%ýÀŠŸÀ7»èc+HƒÀ9 »åô»ÿ@'p0?@Z"{$c?ŋ-ۅwN?àQµSGP@D¼­šØ^?íå¢^±‰?ïßï¿@P¿àö¨ž[¿àŠN½Ó4Æ¿êd†'UØ¿ð?ïõò`L–UNASNone3FGL J1809.2-2016c?âTŠ¯|L¡?Û`®*<à?ÛVê¡f¾?Û`®*<ß?¢xí?½ß¹ŽgÚ]?îØq.®ÎÇ?½ß¹ŽgÚ\?¸?úuÊ΂?§7€_†S?ìø±F¦/?§7€_†R?Æ<Œgì?ERW|­­?ïÿYÎœÈ?ERW|­®4FGL J1808.2-1055?ê•ö– åæ@¿ÂÀð À9 Ô ~$ÉÀ;"ËêN½Ó@¸Á'Z@@ÀA¤>?Ò;"ÀÊ5?éXV£zÃë@"XýÈ[@ëLk'?ïÅbu@ý¿jØ»dç؎¿éÍd1Xh¿ìõºAYç}¿ïÿÿÊPË?ïþÍeyUNASNone?Ðòp;Â˜?ËYïÉÔ"3?ç†Çâ9´?ËYïÉÔ"3?Å鸩?ά…O"ƒ?ꅑÿ•¿ú?ά…O"ƒ?×4³ßB`?ºßÙp`xÍ?äe¦^ñP?ºßÙp`xÍ?°ÿàÌM`ì?¢m!îËå?íàævSâ?¢m!îËå4FGL J1808.2-3005?º ͏´'Àd¤L{ÖÀ9âOOÉkïÀ;oÑEØQe@« ¸qÌ@É$¡ŸøX?̀–Rè/?ÑD¼@àÛwŠ{@žªfpwa¿å¶PôåË?ïø曪ëѿ僲ýmÔo¿äØ=‹ü£¿ë©n*¿ïï¢OJÀîUNASNone?à Šn &©?ËCÃ	e±?ß¾ë#¿²®?ËCÃ	e±?é÷ˆHft9?Íߜ5 Ÿ0?È!ÞÞf/?Íߜ5 Ÿ0?Ýt)P¦6Í?»âú£[!X?áEëW¬ä™?»âú£[!W?åØúß.?· GRtÒØ?ÔOÞ
A£Ó?· GRtÒØ4FGL J1808.4-3358?ïÚ;,i$mÀæØnÁ~»À9…ëOnÓÀ;ÙJr'@pޚՃÖ@Íþu¼D¿?ÀN¢dïBî?éV؉™qV@#4h‡¨ÖM@ð™/¼[;?ïõÞs¾=¾?Èz Ûmé¿àEæÉÎË¿êøToÃÝ:¿ïÿ¥'(^?îK]@ÍЃUNASNone3FGL J1808.3-3357?~Eۋ?ÆýÕ|ã?ïÃuîHéÐ?ÆýÕ|ã?')nÞ$}?'MUº9jŸ?ï·ZE¼‡n?'MUº9jŸ?£d-[ãöV?–¦a~lÜ?îɽ*AÀ›?–¦a~lÞ?*{gå+'¶?"èÐëÒ^??ïþXI­H?"èÐëÒ^?4FGL J1808.4-4521¿ãûØvHùÀ'úƒBØÃÀ:>ýž%ðUÀ;ëø§F*‡@Öáü3í˜@á՚ѧþ?Í»{Ep¢?³š¾‡ºŸ?æ^æªÄdH?ÿ –˜³?³?¡6ÿ½Ý=*¿é†väÝ¿ã@+~³å¿à)¡N™Á¿ïúîéWG¿î?™UNASNone?ïÏ
ëÀkÙ?~ÚĘá€y?xzŠÊ—?~ÚĘá€w?HX<
?"Rñ¸V÷?€Õéðüœ?"Rñ¸Vö?íñc	šI? [Ò_r?°tç´-º? [Ò_r?Q¼+?†J¤ÔK¥?œ¬
5Èzª?†J¤ÔK¤4FGL J1808.4-3522?Ï$][–½À•–\Î70À:ôj{žÜÏÀ<aÏ'ðà@@W¸"Ç?ú«»Š…) ?Òt¡ýì)‰?èÓ €étx@
†ݒî@g*÷O'I?ïù'áê@P¿íßRáNd?ÝÊ®›¤6¿æÄ}ÈØ¡¿ì•à<Z¿Ö×¹ºÌD<UNASNone3FGL J1808.4-3519?ïtMu˜j?æۗê·8?'vQ_ìòÁ?æۗê·8?î¿>.UA?¼ƒEäãÁ?¤«ú?¼ƒEäãÁ?æ¸ÐRæþ?¹}Sì"ú³?ÓðŽ_Z2?¹}Sì"ú³?ì´*73Å?©ÃÝÍ*ô?º^¯öFaÕ?©ÃÝÍ*ô4FGL J1808.5-3701¿î!hÁ¸­lÀ \¥ß"9çÀ:%а‡éÀ<Ö¿•@raÆn@«ñ'l?Äær$àŠ?ÞÿÛlø§@'c/@ñÑHÝi}?難¥¦V¿´'¸N»yé¿âÁ' ÿT	¿çaÃ3ÆÖê¿êYè©¢%Y¿ïþÏ´ÙéUNASNone3FGL J1808.4-3703?'l¹×)ûW?©,Š©F·v?ïtš1F°%?©,Š©F·v?¼ÛA"4œ?ÁØxËGH?ìd—Íû¹m?ÁØxËGH?®¢z°¢ô¨?¢›Ï2Óú7?îØTõж?¢›Ï2Óú7?Ãoo]aè?¤žYܟ¯?ë$$(§…Ý?¤žYܟ¯4FGL J1809.0-2853¿ë¤•µžÍÀ­Š—ž×À:]xFÜ]À;އ$L£@v ís`@è«ÕÜ@?ÒíýÐ?梐MÀ}3@ÃèPïÝ@%&¹Óø?î)<7B·¿Ô€ûþh¦2¿à°ž~蝿æ¢CŒFÊÀ¿ïÿÿ)@k*?ìôí²öaòUNASNone	?«¬mÁ։J?¸´Ü±°¿?îE9#â—l?¸´Ü±°¿?Öè£j¶Œï?ÔãE¿??䋮J¤¹ˆ?ÔãE¿??¼mdò™c?¨`Èlڊ)?ìrSa¬Óž?¨`Èlڊ(?Á¨e½ ´?¯v¥†ç Œ?ëU搗Ó?¯v¥†ç Œ4FGL J1809.2-2726¿çMÖª{]ÙÀÞ9ܚ À9"©³`ëÀ;32¯È@ÕÜÔVÙÖ@w¶ :‹?ЛB;8æ&?Ê扷N``@
Y*f—@MŒ£ ?ïûÏ^¢wº¿ÙEíÊ»{¿è"d~.Ú¿ä-œ»	h¿ås°Á©X)¿ïÿýawUNASNone3FGL J1809.2-2725?ê—Ðô¨º9?Â^ƒ*ô²?Å ¼-]?Â^ƒ*ô²?â†7ìqG?ÔÕ¿›?Úó&ßs?ÔÕ¿›?â3UŠŽËÙ?µ­:.h—?ۙTêâhP?µ­:.h—?Ø¢°)÷#?¶$;u¶ø-?㮧ÿko?¶$;u¶ø-4FGL J1809.5-0816¿Ô·YÌuàA@¥ÊÞ¶]À9gÙÛ©¢À:ì™+µ@Ꮐ[@ôØý\·'?×T=ø´?âÙ`.@÷ñ"íjÒ?úe–w¦)Ë¿·ZŒhƒ¢?ß:…\ '¿êž`lQb¿ëÜÅ}Î¿æÈ|`x»©?ÈäD˜`_UNASNone?Ö"JW?Óôƒ^ñ¬?äîú{ÚÕ?Óôƒ^ñ¬?Ñ)0ÎÈZ·?Ñ	X…yÏ=?çkg˜›Ò¥?Ñ	X…yÏ=?Öî	#Ö"?»(—Kh<	?äˆðûnï?»(—Kh<	?°ezëœ? ©ÂÆq/?íÿ³P¢ŸM? ©ÂÆq/4FGL J1809.8-2408c?ê×<$2'ÀDÍt'yÀ9$«Ô.ÁÀ:{Åyò4e@;€3ìì@>üå™Lm?Ñë>|è]ø?ã¤WB‡'@d>mùÙ?ýƒåîy¿ÛO[²Ù1¿à¾Ûrþ¿çŸTžè¸ç¿ëXÚϐ¿ïô…¾Eu€¿ïüø^KòUNASNone8?Ä[åÙhj?Ė@Oìr?êû鉥å?Ė@Oìr?ÇW:ýîÚ?Ï01–^¤l?ê?ª1@"J?Ï01–^¤l?Éùeúná{?°¥Ö@sl?遦dG¡?°¥Ö@sl?wÇó ¶Â?dR°žô·?ïÐq¾'?dR°žô·4FGL J1810.2-3054?âšÝ[J‡OÀfù3]$žÀ:{ç¨ñ%rÀ<	0pá¬@g0{óÁX@D'¾‹Áj?Òٛ\'R(?ë¬<Ԝ¤ç@Ñ÷ÿ€~@@ŽFø7	?ï÷`‰­"L¿á1;A®A¿µù3¡ÜÍæ¿îÇ[¾í'¿¶",maZ¿ïÿѧ' ÖUNASNone?ê1Dåú?Å®A›¶Õ?Ǜ:ìhß?Å®A›¶Õ?åƬõÌ<Ã?Óûãज़&?Ôr¦g†{?Óûãज़&?ۂt¨Õ?»)¿kQ@?â>þÅû«–?»)¿kQ@?Þþäeu.Ë?ōžœÂËp?à€ÍEh›?ōžœÂËp4FGL J1810.3+1332¿ï`_50 @.A•övêÀ:eÜyhÀ<¤~Ïé¸@iÑãâèî@k;¸<òÐ?È÷èÔë?Éٕ2+Ì7?ÿ¡Ž«)?ù½X›L¢? Õ`¿â4Šˆ×¿âÚìJ@•ò¿æ¦]—ŠË ¿ì¬…dXo-¿ïÿø¨ó©°UNASNone?èM!Ï,-?Ä/ØÉ·W[?ÎË{ðÃOK?Ä/ØÉ·W[?ädŸ¥)˜ƒ?Ð[À`ð?×6Àµ¬Îú?Ð[À`ð?è6'þä?¶-BFd4?ϗ%»äq?¶-BFd5?áÑ@0«Á?³Ö؅Ԓ?Ü]ž©Ê}?³Ö؅ԑ4FGL J1810.4+1700?ïñî†)$û@0ŽÓǒÑ(À:l0 ±»ÏÀ;ÇVpOu@™¾JÓãÂ@Þ?©c;?Ñ8š{@èþ?ÒþÄt¹@b¼ºh?ú[oó¯¿ï¢36ÌE?ç†tX—pÊ¿äÜþޗÐl¿éÌ«ßí;¿ï°ÿ笿ï^­À1ËUNASNone?çc¬ç£?ÊO²¿e'–?Ñ8¦1Çî¹?ÊO²¿e'–?ã& ܇8?Ó~ÌÐ$¾Ë?Ù³¾FñՐ?Ó~ÌÐ$¾Ë?áŠM–:¶i?¹ZÚԊ?Üëdӊ".?¹ZÚԊ?×ÀñódŸm?¹¾35RÌ^?ä‡M°J?¹¾35RÌ^4FGL J1810.5-1415¿ïÎTg×äŠ@·|ˆçš®À9(ê°£À:ˆ¿™Þb÷@ÕÒmrÊ@ìbÿ©˜ë?ÐÁ˜ÜZ^p?Íîryo,´?üQ*"ÿ&?ñ?ƒxšñ]?ïb´•žbV¿çWy-éGW¿ë:§0[Ÿ¿å+,Ôt`û¿ïÿü¿ÙŸC?ïÿÊjåQUNASNone?è´T¨ð?ËKöMÇ:Ã?Í.­_ø?¶?ËKöMÇ:Ä?áÄ.sæ)?×ÌõlL
?Ýðw£3¯?×ÌõlL
?ák¦×û܉?µ¾ƒ{‰¦?Ý(²PFï?µ¾ƒ{‰¦?¶¾êe‰é?©4'憭?í(<³NÃ?©4'憭4FGL J1810.8-3347?î'móhÀVAb ßÀ:<piõg À;¾9ìN@ád^y]@|ªu‰ð?ςe"oä?Íöc7‡×@œd…D@³jÑ?¿¸v×LØuÍ?îx`äÇ?¿äxrØd°"¿á,|Ë,¹œ¿ãúÍ[h£¿ïü½Í«oUNASNone?í2­TZ{?´Ã$ôÀ|´?·žj•],+?´Ã$ôÀ|´?î,F¤MMJ?¼f‹—å?­;•»++u?¼f‹—å?è€6 NFž?³«PŽ&è?Íÿ'~ÆåŒ?³«PŽ&é?ì:%ü?¥S?¾¡0?¿¿þ.Óx$?¥S?¾¡14FGL J1811.0-2725¿âSŠ7uùÀh"!'÷¿À9ëˆêá‹À;ZÆü©3k@Þ´\"~Í@vœ©ïR3?Ïx´‡0¶V?;:bÒ]@rpŽ@*;±±éG?ïّG=V¿¦©aD¿¦SÛÓ¥Ú¿ëˆÎ™«¿ÖЀáf⸿äoTˆ'UNASNone?çó[dÊV?ÅÃNºâ?ÐHå6kR?ÅÃNºâŽ?í³µÅ]¬ö?ÂI4•]^—?²bQÕ˜M?ÂI4•]^—?äù
3%E?¶ÃW$÷?Ö
Ó뙵v?¶ÃW$÷?éÏà‹óJœ?´üž/ó?ÈÀ}Ð2Ր?´üž/ó4FGL J1811.7-1442¿íêE7æ?þ	üD}ÞÀ9ÖÄÍ$À:ÿöÅĚÏ@ŽEµì¶w@Ã%Nn"?ÐýGþœ?Ùp ¤eP@è%@+i:?öcˆm¢Dä?ꐦv î?Àá®Ú÷³¿ÚڞÜúlm¿ä½ì)‰fF¿ì?韖]пïôÞcβUNASNone?¦§ë´¾°?¨¹Œb·al?D´ö?¨¹Œb·al?öε£?˯¨«"\?ëLR¸9?˯¨«"\?̆fæƒ?´§Œ_÷M?èÞz}æF_?´§Œ_÷M?¸\0]& ?›§Çd9J?ìôyô],?›§Çd9J4FGL J1811.9-2336?҅8f,YÁÀ¬|•|ÔgÀ9\Úx†ú[À:¡?´‰	@ð"댫u@e€éŸk?ӓI]ìð.?áK.g˜@Ê÷	·8ç@g|"¤b ¿ØÏ[†I¿Üw†´º‡P¿è7¾³.–¿ç©ÇÁJ¿ïÿûÎBÓ?ïCÿ3QfUNASNone?ÉÈ-+T×)?Èrõ†àx?éôµ*Ê5?Èrõ†àx?Üíb'–¨?ՍŸôël?á‰N¾´ô+?ՍŸôël?Ð_VÍÍn³?´2‹Ñfd}?çÐT™H¦?´2‹Ñfd}?Ã.Àá?²QXt¯ü?ë4OÇ»ºy?²QXt¯ü4FGL J1812.2-0856¿®³xÖÝÕ@ãâ"À9iÀv}4ßÀ;…nij'@I†¶º'@{©f–7?Ñ3a×5†?éU—¬Y¾@Ót62Áô?üq˜ç%á?ïðdìé¢Æ¿ÕUÕõjzÈ¿é®Æ¼èS;¿ïÿ–Aö¿è»À½Iø¿îQ9]ïŸ`UNASNone?Ó"*Ò²ô}?Д"Ù)ð?ænꖦ…Á?Д"Ù)ð?¢Í¸.c/?ºŠdp"P˜?îÓ$}Ï­?ºŠdp"P˜?ÖIÕ¶iDÑ?¼°D£3À?äÛ$Ë]˜?¼°D£3À?e´—@*?Y"&3¸œ?ïêKøh¿õ?Y"&3¸œ4FGL J1812.4+4441¿ï­3ĦÏm@9TgÓMðÀ;N'™ð×nÀ<Ž˜÷³*d@yòŽÖr@ ؽ›×a?ÇbY&D¿š+WÅ®K?Ó4ý¾1@ÊæÞpä¿å#ãŸw),¿Ý$	_$RÆ¿èr¦äÌÉ¿ÑÀWs"\¿è™\þØ<¿ÔðáxÚUNASNone?ïÝcɊé?lÐd½ýï?qNp›:ŠÙ?lÐd½ýî?ïý¨ÏLÃÁ?Vçäí÷Jâ?2¹…™áû?Vçäí÷JÚ?ï¡Ù`8²?†ó·]pg?‡‰§ñÓx'?†ó·]pe?ïî܂Ѧ?QFSDóš?a#}÷.Z¡?QFSDó—4FGL J1812.8-3144?ìj¨?ðüÀýœk1˜À:'È-*ÛvÀ<0æl±C@Ž!AÄ¢?þ_æðd'?Æz>ŠJc?à·l³‡i@þ•`Nõ1@')ó?ïÿæj,Ą¿ãšÀá?µ¿Äx@Ùd	ë¿ã,æ³'à¿í…·š5 Ì¿íؾópPUNASNone?À[ˆAŒïÉ?¿	œtš@?ëéïœÄ
?¿	œtš@?µÙ#šnç?¿ä=u(×?íDÎŒ²#?¿ä=u(Ø?³ºVÀ>,\?£(£Qþí?툵'ø:u?£(£Qþî?‰1°¡ö)?¨óAwÔ¿?ë]³"ׂv?¨óAwÔ¾4FGL J1813.1-1611¿´¸÷óõö?ë@dïmâÀ9.ð®SeÀ:J£Üºî@øÓ4ð͈@i:Áœíâ?ͳðÈT˜?ÀVT_þ˜L?õ-ŽxÔ'4?Ø٘,‡"¿ë³Na	y?ï2a|ÚQ¿æÙþäw
~¿äHîៗµ¿ë¨a}ÉY{¿ï¹úݬCUNASNone?Ô[Ï®ü¾?Õ=æsº3?åÒr¨ ?Õ=æsº3?ÑH]kŠ?օš$<SM?ç[þÿQJ:?օš$<SM?ÝÍgUÙ;?¹¡Î96	?áLUzb?¹¡Î96?ÓÉÀ—ç?Ûêü ÝÑ?ïa±ûGÉ?Ûêü ÝÑ4FGL J1813.2-1128?ì&E9a‡ë@Ȑã²°À9.@q	W˜À:¡»á¸@‹Ò@MM@SÝͦ?ÆðtöL?Ò}PbÃï"@ÇÅ&^?éÒ°;¾ê?ïO+.?®¿á<W3Ã{ë¿æÉvÁ}cX¿æORîº]^¿ë€uf¿ï³Ñ¾¤UNASNone?¾üX¶1µj?έWÓi¥?ì té9ÉS?έWÓi¥?¸Öqýû?Çôá®:#?ìå1À\ Ÿ?Çôá®:#?ÅZìjIB1?®÷‰¥†-?ê©Dåm¯t?®÷‰¥†+?qéÀ1¯G²?^Ixâ—?ïÜ,œ¡q?^Ixâ—4FGL J1813.5+2819?Ыˆ±y½×@41ÿ?àHÀ:Ý\úŽ§À<­½MÓÈj@Püi¤&?ûޑÖV¹J?ÌðÔ¾Þ¢?àM´ôhó	@jÝÄkÕ?ôÐÓÇè·d?îßÛgšC
¿ãç- I¡Š¿Á瘋§"¿Ü«´NPÅë¿êtÝAäüÄ¿æPazChUNASNone3FGL J1813.6+2820?Û-±íDZÚ?É ÅYkƒ?âi'	]Ғ?É ÅYkƒ?»#"ê	?Ê2ƒ¸‹7>?워Mb¾Ý?Ê2ƒ¸‹7>?ÐßÖj~G?³äGŸtE?çÊÀÜq?³äGŸtE?À"r¼»C%?¥®9&\"
?ëÚãPÑ/6?¥®9&\"
4FGL J1813.7-1152?æã"îwþ@IÅÓï×À8—¡Vý<×À:I">¿@0êp ÏX@3¾sm¶?ÆZ"Zî
9?ÆkúdŠ™!@D,Ý®œ`?ø9€=Òô¿ë@tdUë?ï^µÍ¬Æ¿åßÁ œ,Ç¿è½^®(¿æ˜~±¶ÆÑ¿ï÷ýO0ÀUNASNone3FGL J1813.6-1148?¼ªKrÔ¶H?Ã<3LKmv?ìj¶'¥i7?Ã<3LKmw?²1¢'<¥%?À|j"…³U?í¹Ë»k[?À|j"…³U?ÎZÇ/Ç?»'Y‡4Ô¨?èyéN?´?»'Y‡4Ô¨?¤\CzÄã?›r@)t"b?îº;ÈS¿²?›r@)t"c4FGL J1813.7-6846?ÙT5Sµ#èÀ5Üك"t—À:ÂÀ<G³"ÛÈ@ȪWVþê@çLû‹&?Á.,¹•?ÉvÙ%J½>@]o¿«|@æW¢Ô*å?ï'È#ð ¿à€Õú¿ßìÐÃ|l¿æÜN_‰}m¿ë&ojñæb¿ïÿö$´ë/UNASNone3FGL J1813.6-6845?áèY¡ãxB?ËÁVQSì"?Ü/L¼9}?ËÁVQSì"?é½Gg{¼å?ÉpÜP6†?É
âbg?ÉpÜP6†?äIAŸÝ?¹šƏ¬?×m}ÚÄÀF?¹šƏ¬?å–Ý j?¯X	Jɐ?ÔÓÆEÊ¿)?¯X	Jɐ4FGL J1814.2-1012?ç™÷_.+X@ÑăR/xÀ9u]ù°Z¦À;§ž?È@†ò¯	˜Z@$Øý\·'?ÓãҢϣA?ïÎÿ!]ȳ@v9þ(k?ÿü¢¯»Å?í½Aߞ`©?·ÔÂ]³¿íw6,â·¿å³:Š?‰ƒ¿æ4á‰t¿ïÿèîkƒUNASNone?»_ä2`7o?£¡6´'?ì"y³ù?£¡6´'?µu
uz+?Â2Ì`"`è?íQ^QP¿?Â2Ì`"`è?Ö²ë?¸ϒ~?䦸v|ž+?¸ϒ~?'³f%½y°?"W÷¶—âÙ?ïrdÎÒ2?"W÷¶—âÙ4FGL J1814.2-3000¿áÌ
õ¨¾~ÀΡáf·ÅÀ:ØC1­÷õÀ<mCÖïe~@0ÒĚ?ü}s]Å­õ?Ô»´4çh?瘒üÕ©@;YÎy@TÀœ<â	?ïýî½ãOñ¿èø¥˜«]¿Ó/ÕÜ¿çpi§Šô¿çg'…€Þ¿ïÉƽ¿ÐUNASNone?ï~(äHÜw?—:µa2ù?:ãväqT?—:µa2ù?ëûrú$ô?Dz˜;k^?À7øl/?Dz˜;k^?è.×èt´?´p£©bë?ÏEø ^-.?´p£©bë?æ˧â¤?µÞj­?Òh±:·È?µÞj­4FGL J1814.4+2429?ÓTW=ó³@22ç³ØàÀ:vÉ5h—™À<‰a=2@'ìðٜi@Yã¡$¨?Ø1#ùÚL?Ó´B|Ò8œ?ÿàç6Ÿ?óDCƒãNï?åÉl|«¿ã¤­><%Ë¿é²¾=èÃοåq؊p0ë¿é+·sŸ4
¿ïÿÈ!ÂGŽUNASNone?ããªó9?ÐUÇÙ÷Ô=?ØáÄ8ªŽ?ÐUÇÙ÷Ô=?ÝÝ#~§ÕÕ?Ô²>}ÖÖ?án@¬?Ô²>}ÖÖ?ä7X	Eʸ?»Pe™sQ?בOítj?»Pe™sR?ЬòЂ?µÀŽƒŸ4?çöu)†—¾?µÀŽƒŸ44FGL J1814.6-3621¿¬U?ÎÞÀ!ëÒRGËqÀ:±šW.ºþÀ<,3øUÔ@dn¾Ï‰?ýAŽXø?ÒKÝcß$?Þ¼Øc@§"©GŒ‡?þ<sÿP³?îö+jçÕg?ï†G½Xæv¿×(èÁõÙ6¿Ë1··¿êJë€ìúj¿ïõXÝç¯UNASNone?î´4ÃUÛ?®Ÿ­ˆÀví?¯D¼³Ê¢F?®Ÿ­ˆÀví?èAɏEŽ4?Ðg']"
w?ÎøÙÂéÇ0?Ðg']"
x?é#åv¢Ž¨?±Ç"0Þï?Ëpj%uÅ_?±Ç"0Þï?äËR´•ˆ?¶êh†-?×ØiZ–Ôï?¶êh†-4FGL J1814.6-2537?ïdˆüåèÀ°LÎå«ÁÀ:qó·ó ôÀ;±rGE8ï@Ï0֌"#@x~…A?ÛÉ{"P?æãèb)•Ñ@ãÈ\$Ä@ÿ[g¯¼œ?ì'1ÆK©L¿Ê™ú<œ"t¿Õyëñ@¿çýB`wº¿ïÿþˆ0»Š?ïÿ£ÿywUNASNone?тBv¿‡h?Ï÷W|	ôó?ç>ÞÄ <L?Ï÷W|	ôó?ä	üÐäÇË?Õd´5f'U?×ì^6pj?Õd´5f'U?ÑIÁVé,?¶…
£Šiõ?ç[~ԋi?¶…
£Šiõ?à…°¹1\?À°Aå;Í?ÞôŸàH?À°Aå;Í4FGL J1814.7-3420?ïVöÒs`ùÀ uæ6*^À:xv3cÀ;Ñ[§Æƒ@®Qäy;Ö@ëE®_ú<?ÑgC:è3[?ÞcK©Í@.ã,?öVwî¤
?ïã&@©?Ô1½|Í°ø¿áÜ4-n¿ç<¢³Ï¿í}Sþ.ïÑržƒ
fUNASNone?—íDJ½ø? <Æ'ä?ï@•Ýª;? <Æ'å?¢)"=»?°=Üã'åÂ?îÝg¼/O?°=Üã'åÂ?²¨¹Š4UT? ½Ã"¢N?íªèιuV? ½Ã"¢L?Xs63TÁ7?E]$×1¶?ïóÆdæU ?E]$×1¶4FGL J1815.1+5917?î¸!'•Ž@;Ÿû¹IbÀ:áZˆâ'1À<D|	f@×lu:(@¿\¢˜F?Ðb\ªŒ0?æ­z¹Â@ê±ý=­à@áð˜XüÆ?ík9i®ƒ¿ÒîÍþ¾a¿è̀†£пêòI^ãL¿ð?ïÿ±%§YvUNASNone3FGL J1815.1+5919?Ø5ñ 3!þ?ЧIqY¶?ãå/æo?ЧIqY¶?Ö._u­?ÔSÎõ´R?äèÐrEx*?ÔSÎõ´Q?ÜÈQÝ
¨?¶†%|· ?á›ôWz¬?¶†%|· ?ÖaŊ";b?À¦…Nˆ?äÏ:½âN?À¦…Nˆ4FGL J1815.3-1336¿àyò|6?ùæŠÁXÀ:µc#»ÇÀ;­iiP%²@h½}¤p@/%¿­*?Ն¼RV9?ï‹'!­@ØÜ@Þ¡@Ѻü•½A¿äúœl²±¿îd%ÿn	É?ÆÔ¨Ž¿äJæ
²û¿ïÿ¾[ðÁŸ?àRâ¥üÿUNASNone?µë¬J`¶?À[gq&Œ?íBŠv¿Óé?À[gq&Œ?ÎhD~%p?Ó~"Vç¬?èeîàv»$?Ó~"Vç¬?Îe»Òì¼?³â½íšä?èf¾'DÑ?³â½íšä?Ë£¨ÕÇGR?¸HUˆ2:t?éʎ.+?¸HUˆ2:t4FGL J1815.8-1416¿ì¾Y§9?ó2±-4À8¯Ö»cýÀ:<òô~Â~@ûèɂ•q@#¼ª ?Â-«3õÐÒ?͍eä@ûdg?ìiZ"›õ¿Ôû¿¾òCª?ëÄQh¨`¿æ9œf¿æ"‰!Q^l¿ïeDþ6ҿ撝'uÞ©UNASNone?²;÷·z"?ÉZ‰"ðڀ?í¿x	®?ÉZ‰"ðڀ?˜Æ¦¿ÿºî?¯ž‰J¤?ï9ÊÊ(?¯ž‰J¤?·í*¼$?¥‡ñ•®‡?í]ú¿È|?¥‡ñ•®‡?mÞW°?\f6IÞg?ïâå!¨Oú?\f6IÞg4FGL J1816.1-3908¿äûèÎ(®ÅÀ$ù³ÃçÀ:Q¤nß±¬À;ðbMÒñª@P‰áÿº@
vÙ{0ù?ÌÂ*7‰?ÐGýûCÝ?ýVÝA‰?ò¨"pÃ6¡?ïýê|
<š¿åÁ`>¯¿åáù£Åm¿é=b.$¿çû¾Aě{¿ïñÁ—ådUNASNone?îur°Ë?²xõih¶?¨¨ÞDþH?²xõih¶?éÁÛ_K½U?ÍÛ|q"ä°?Èø''Ñ
®?ÍÛ|q"ä°?ç8Ô~Íª?¶ñv0Hx?юWàd¬?¶ñv0Hx?Ýtlü‹-'?¹a?·,?áEɁºi7?¹a?·,4FGL J1816.3-2903¿ïæó£­óýÀ"ͅYÀ:"Ü·%››À<opŸM8@*ÓÄ[d@DEª.<?Òäç`Kð?ïÿûÎBÓ@Èd©ÍÄ?þr¥;¹>¦?ï'v1µ"²¿ãýô·ø¿Ò™#"™Þ¿ïÿâ£Î¦Â?ï؊p0ꄿïÿüoQÇsUNASNone?ë¯"ð§¯?Ê@6Gbƒ?ÃéA¬=aD?Ê@6Gbƒ?ãYhGUú#?Ø¡O×i²?ÙM/qT¸?Ø¡O×i²?ÕÌ2ÂÀUd?¸übZ"?å枟ÕN?¸übZ"?ݹüã{?Òhª©Í7:?á#öŽBw?Òhª©Í7:4FGL J1816.4-0057¿ïC‹jº5@_¾vÈ´9À:.Hè§À;_WƐr©@ïxŒÙ—¶@ˆ¹º¡Q?Ìzº0gý?Àÿìý)·?ö©Ä¿¸T@WKÐ
!?ÜA œ,ÆÝ¿æރ¾ôÚ¿æ¢:Að:e¿ãøèI*}¿ïüŽ[wõÛ?›^L€PJUNASNone?îz'ê
z?¬÷AðU¸O?¨Vá^ÿ(^?¬÷AðU¸N?íí/¡Ÿò?¾át†¿Õ?°—Þ'ól?¾át†¿Õ?뵒<|Jf?«o¯·Ó?Á)·Öd?«o¯·Ò?îp]ñóñ?–­…d?¯8ú àÀç?–­…d4FGL J1816.4-2727¿°ŸÁ
‡""Àªä>šÀ:EžG~CÓÀ;ÕbþÒÙV@týۅ¢@58[' N?Í$ɍþ?à†ü©3j'@µÇ`c?ü÷Ǫfp?ïœQքܿá÷ ¦éŽ¿ãƒ>
É¿ÜÔ»%_¿ï
•µŠé¿ïÿÍ'ý UNASNone3FGL J1816.2-2726?©vbð$?­éRE"…?îhž¹Ðþ.?­éRE""?Àl rõ‹?Æ•›Ýì?ëä÷ãzBž?Æ•›Ýì?¶jYâÐ6?¤,ÑZÙ?í2½"Ã¥ù?¤,ÑZÙ?¡JSʁ¯?†Ž%Cd´O?îëZÃWïµ?†Ž%Cd´O4FGL J1816.4-6405¿ë'A‰*B\À4ŒfçÀ:V#ßÙÀ<FÒä>@$þØ;–@›¸€®?ÀÇÐy)·‰?Ö°Þ$
%'@÷jøœ^p@eÍ=`Ó?ïÞâ¾ÑŒz¿ÜTµ"0ѯ¿à€ÎۚƿåÖ½•!e¿ïüK_ÏÉV¿ï'nÂ6ïUNASNone3FGL J1816.0-6407?Ã35l"Æm?Á×sçÔ?ë32¤ÞÎd?Á×sçÔ?Óôyp©%¦?ÑüQJ?t?æÃG«m-?ÑüQJ?t?¹ÜTˆ>‹?§8T¨¬çÚ?ìÄunþ˜/?§8T¨¬çÙ?ܪÎç¿?²Âž©-Êë?áªü˜Œ ?²Âž©-Êì4FGL J1816.5-1208c?èœ!ëwX@Š	¾Å£
À9>'lVjpÀ:¡¨žð@þÓ xñX@!Äüó0?ÌòÇÞ%²?ËáÌ8RVå?ú€yK!@»t_οïòbüO?îþýÁ·Dû¿çIðäÚ	Ì¿áÇr_Ãßé¿ì|vÕIs¿×8\OUNASNone ?Á8Ú¦v˜ã?ıӊÜ?ë±ÉVbYÇ?ıӊÜ?هïBJ?Õ4¦.ûÙe?ã<^ö?[?Õ4¦.ûÙe?×5–Ýkü?¹(®~Rv?äe4'Jpƒ?¹(®~Rv?áàŸÉ?Ÿ?ÁãGö̯J?Ü>ÀmπÄ?ÁãGö̯J4FGL J1816.7+1749?Ë>ùäõìA@/M߆ã´À:GI¡À< SúSÕ@@ƒÊû;u@XTŠ›ÏÕ?ðHÔÛd?Ðv	ý.êN@OÈ‹ñ:@¬ß¡GŽ¿â-ŸàÛwŠ¿ÝAÛ¢R¥¿¿ãßKà(IJ¿ÕÎN­=%¿î«A—z©¿ïáØݧ:—UNASNone?Ô	<
¯€?ÅR#&ô$?åûaüy(??ÅR#&ô$?âôRÄHÒÂ?Ó=m[xm~?ÚZwnZ}?Ó=m[xm?ÛjVâ˜r?ºG¹‹D!?âJԎ³Æ¿?ºG¹‹D!?æÞUU$*?²¬~ƒ¬ï?ÒCUU·«þ?²¬~ƒ¬ï4FGL J1816.8-2800¿ßéˆRàÞÀq´xB1À:fVߋÀ<
çbzH›@ë\ђ.@ý'$ZR\?Ô¹A?:}?ï¬Zœ-Ȑ@ &5?þOL'S$¿Ç"(GÔ?î¼ZYê
¿çoÚ]ÙúÞ¿ïӃüº{?êÿ}úâ~¿ïÿ:Þ"_¦UNASNone?àzŠ¡›í{?Ñ+x§lË?ß
ê¼È%?Ñ+x§lË?æl¡Ü.Ó)?Õ¼|Œšc?Ó&¼G¢Y¬?Õ¼|Œšc?ØâW‹vœ?»Ò{+Öj?ãŽÔ:|IJ?»Ò{+Öj?àO©+mƒ?ЋEQù\?ß`­Ù©$ü?ЋEQù\4FGL J1817.2-3035¿×‹xɃN¥Àœ…×EÀ9oßq?RÀ;¸ò–Šñ@Øä|û@؛7(‹?¶¢bk/å?¯Åäü"Ì?ö-$[)'@²¹c
–l¿ÞBkØ?ïÿɯæ¿æ-'?2D÷¿â§Òw0¹¿ä³!96¿á'‡N={UNASNone3FGL J1817.3-3033?ïÇgá$oP?*)z½Ûô?|LmÈWÊ?*)z½Ûò?ïÚ;­¥ ?'TNãM[?râ)-@p?'TNãM\?ï!ñ
Hð?•Ëöy½®
?›ÁÞ¿6â?•Ëöy½®?îŸ*js?"Ã3yNÈM?¦YXΝ?"Ã3yNÈM4FGL J1817.5-1034?åþúÅ«·?@³	ý¯Ã¨À:ÇíiûFÀ;Ù€9vC@©Š(b@ñ]¥Í"ƒ?ÒáO¦0€Ñ?ç»ÿTßUf@‡0[žŽ?ö7–§¡Å?çèQBgك¿²ªËÁµ¿Ö§e47?1¿ìm² {¶¿ïÿþó…õ?︣µ|N/UNASNone?´î
õÂ{?¼Á›¥öa€?íb>A\Ç°?¼Á›¥öa€?Ð!£ÒÖVø?Ô¢bo
;?çï."Ôƒ?Ô¢bo
;?ۄÁ E?®Þ¶"+?ëÏ·î½?®Þ¶"*?Ž—A~?¥S?r8nH?új?r8nH4FGL J1817.6-3251¿ÎÈd¥1ÈÀžm=ðüWÀ:Ò7yêÀ<€Èþ3:@hÆøL'e@ÛÈ:–ÔÃ?Ö¬]᲍?ïô×x!yÍ@'ƒ'à@_VlHS¿ïöë¹÷Ýó?ïÿÄ;-Óx¿Áí@	Û¿íO9ßÞè¿ïÖ´!…5ß¿ëœm‰pVªUNASNone?ÂÊM"·™?Éš1":ï?ëMlšÒ<?Éš1":ï?¿8Dö7Ç?ÈE–êwC?ì÷a9?ÈE–êwC'?Ì«ÈlR])?²ÌËÅ¢|¹?èÕ
äëh¶?²ÌËÅ¢|¸?"êëx†?{pGS?ï`¯À¤;Ð?{pGS4FGL J1817.7-2517?íHS÷QÀª0À'+çÀ:–kÅJøÀ;¾}ík¨Æ@‰+Îdý[@º"¦6?Ö<€"Þ?àþ!†ù"@
X¥ÛÇ;"@‹4ԝü€?ïç¥*ÇSç¿ãe•®×ï¿á˜aÁ;¿åzJIˆà¿ïÿÿ" 5•?ïúµK¦ÇUNASNone?çÓ¯æ?Ëä'Üð¡?ÐY÷Ò 3Å?Ëä'Üð¡?æXø&á?ÓþÛ*†ü?Óû÷N²=?ÓþÛ*†ü?Û{¨«Yžˆ?Á"t/$?âB+ªS0¼?Á"t/$?átNa?À·ÀzÂÐ?ÝÇÕc=È?À·ÀzÂÐ4FGL J1817.9-3334?×bZ]
ÙåÀ 'ҝÇ%ÄÀ:Ø"r8À<(ÐV©Z@RȲ5ò«@–¦ Z?¸m]ôþ?á¸W=Ôw@ 7 þ}I?þÀd*
ñ?ïþÎ!`¢Ø?ÀÄ,[Ø¿ÝÿFÃ*¿äu/dÊ¿ð?ïíßlÁÕUNASNone?ƒÄÁ¥t1f?'±ÿÀ"­?ï°ìùj/:?'±ÿÀ"­?™$7ÿ1Ò?¥$A‹¨î?ï6ÞDr?¥$A‹¨î?®Û78x˜?£0ž±Ïø×?îFüŒxw?£0ž±ÏøÖ?O~?tbèþŸÿt?ïºÂ³ß?tbèþŸÿt4FGL J1817.9-1135?ï÷g ßVÌ@+àXšËÉÀ9H¬A<
À:ºŒã¨±e@]ÆYÁ@ßú¦ú«?Õ4<Ëbj?à÷–oB­ú@
ŒWâ?$Ù@¦o¾(ð¿Ö#IüMmò¿Þz"@Ÿ¿äkŒ–|¿ê¹ÂÅâοèkœ0LÏ¿ïÿú¡œGtUNASNone?ÍÁ¬;°Dÿ?Ê¥÷4¡Õ?菔ñîÁ?Ê¥÷4¡Ö?ºÅÃö[a?Ãáäù›b‹?ì§\G4"?Ãáäù›b‹?Ñ0 H×0ß?¶<d­VÖd?çg¯Û"g?¶<d­VÖd?º8GT£R'?¨'²§í\¢?ì¸÷k•º?¨'²§í\¢4FGL J1818.0-1339c¿Ñ8ӏ-Ðò?ðWš5 Ë½À9?Ùx¬ºÀ:ZaՈ@­>'
@¸©õ1?ΟH/Cºj?ØZí!*È@‡#uP@î›×6ˆ'¿ïæ†|†c\?ïú^À՝¬¿à³%³A¿æ
ŽÏ;<¿í<ÜÊpÑú¿ïì¼Á¼ÎRUNASNone ?¬|ªÇu?À±\rl‹?î85Sˆ§ç?À±\rl‹?²'²«Ü­?¾ ¨ŠB¤Á?í¿mɪ"j?¾ ¨ŠB¤À?¿Ç~BÆj?ªTvmÞì,?ìp7§3?ªTvmÞì*?Îò#\êî?¶Ø7Åzè›?èCx7(ÅE?¶Ø7Åzè›4FGL J1818.1-2000?ٟ`õÅÀ	 bvÞÀ9æk¤"ÈŸÀ;Æ¡Ú°»@)²~AúK?ÿ)¢üê³?ËæáK	Î?âÕm…>˜Â@)4AP,h@ŸJ(Åò?äT´W‹P¿è4%CâX¿Ês4j•Ë¿ÓìöÖBL¿í#¼Sƒ¿ïÿ·`)
UNASNone?¸×ÑQ¼?ÁRÄÓû‹?ìå\¥ÕÈ?ÁRÄÓû‹?χà"–[?ÑÂ]ì÷í?è>‡ÚÚi?ÑÂ]ì÷í?ÆxWlË?´ãù‹]?êaûº*$Í?´ãù‹]?͞g;øëo?®ó$úDzö?è˜f1Å%?®ó$úDzö4FGL J1818.3-1233?å+UΘ¸?÷Û¼Ú'.À9'0¤ãy·À:¶]këáe@ G9Oó@ݙÙZyÉ?ÊüÑâ¶C?´Æjˆ	#j?îXþý–ï?û´¦xz:¿ïç܈+³?ëÍ$ Ҕ?µÖR²÷¿æ­
$F0f¿âù!°:¿î³©æ÷UNASNone?é[ÞŵWy?Æ©Kðr?ʐ"é*¢?Æ©Kðr?ä+:¨ÁIR?ÖR}zN…×?שŠ®}m^?ÖR}zN…×?å×1!@®?Á@'g"¾µ?ÔQ㝽~¥?Á@'g"¾µ?æ:-GÛ?½@µºóS0?ӊýÿ¥pJ?½@µºóS04FGL J1818.5-2036¿±â+Â?ylÀl²
.À9ŠºÅ­À:Š@aïß!@
uΎBù@¢ÍbJ?ÑEäü"Ì?Ð0üw?ùúYÍÑ°?û輻@-?ÑE0¡2•)¿ç.yÖ¿èÿat¿ì<ø¾îì¿Û¦¾%6™¿ãi¸ËŽlUNASNone3FGL J1819.5-2045c?ç
o4¾?Ë8ž"=¥‹?Ñå!ï—ʃ?Ë8ž"=¥Œ?ìÙ[Tçvi?ÃÑí
;?¹5%XÄL²?ÃÑí
;?áËn+m?·l¿(m?ÜiÏ#©%á?·l¿(m?åèvJX?ºÖ"Ú͗\?Ô/kNýÇ?ºÖ"Ú͗\4FGL J1818.5+2533¿ìœ‹}ïÝ@2$Édb€(À:>"i®ðCÀ<ôËÛk@ƒ¸x¬äû@é/n'"š?ÈHLŠr4P?ҋÃbjÙ=@ޓ@ºs@Š]sùvú?äþÍûÌ¿à)F Mgè¿é±'IC?ñ¿ç-'àAõ¿ì`½¯ùWo¿ïþV²"<cUNASNone3FGL J1817.7+2530?è:ézØ0ù?Åw!zÍo?ÏZŸ<?Åw!zÍo?ì¾|ߋbX?ÃI•%\?º¤íB?ÃI•%]?é
D*R?²¯Xgö;Ä?ËËïŠïV¸?²¯Xgö;Å?ëðzt 9V?¢~ÓiõI?À>/ª?¢~ÓiõI4FGL J1818.6+1316¿í@üc>Ã@*fZUÖÀ:h«=0À<€à,@ÐøÇÒg?þ7Tð]?ƎNâ¼"[?átÝ!®¦q@mÝS,Î@¡ÀM|€?ØîBþ­Dœ¿Üô[艿ЏÊB®Ñ9¿á›þÝÁ¿ïó6>¿ïva0FšUNASNone3FGL J1818.5+1320?°Ñ	#–X]?­Ç,
nh?íåÞۍ4ô?­Ç,
nh?ÆÙÿ}ê̪?Ï·º| ÖQ?êI€ …LÕ?Ï·º| ÖQ?¿¿h3$Ö?ªXNf¬?ìù›}?ªXNf«?Ï{àYˆK?«•H€»
?è!:‡éî?«•H€»
4FGL J1818.6-3206?çïOt?ÄÀŒ†‹ŸÜÀ:#R©@À;Ûo¼P}Ç@—%'Ænd@˜{0›©?ËJ3•XÂ9?âîA'šÈ@å	9d¥œ?ÿiÅHŸ6?ïÌ¡-â'Z¿¬ñu?
e¿á±Îyu6ä¿è™¨èÁõÙ¿ïú×lbÿª?èøª O€ÇUNASNone?¢·¿x¼?¸Ì]¶í¦¹?îԄt?ç?¸Ì]¶í¦¹?À+ß6ÑTc?ÈfÂìº[8?ëõ2Kªç?ÈfÂìº[9?«0Ìx½M©?š¤Vés±?îLó8t+&?š¤Vés®?£¸"Üs1]?"EîV7ì?îÄw²8Ìé?"EîV7ì4FGL J1818.8-2255¿ì
P#§Ü¯À0U¸™9"À9×	—XvºÀ;>|2€…Ì@š¸ý·ü0@÷GMœk?аiϘ?Ò «†+(@wºÄŒŒk@¶¤¬È"?ïɯa!¾¿ê~Åý0¿à"7É
û¿ãÁ9ñ"U³¿ï÷Q۔欿ﴟ¿x{gUNASNone?éÉ?ÚVÀ)?ƹÞe÷?ÈÛ–¤ÿX?ƹÞe÷?í6À_ëg?£Gc+)'?¶Iý¤Ç?£Gc+)'?ã²Ä1¾?µ<gá
R?ØÅæšwœ…?µ<gá
R?èöÍ+|€ã?¬9¹P?¯‰?Ì$ËR
üp?¬9¹P?¯‰4FGL J1818.8-0828¿îiýºó8@
\‰ô
(xÀ9e(ÃnÀ;=ˆ ËR@¹·_­@Sœº¶?ÇCŒ^?Çãv‡pÍ@7}_§/"@"؊ñ
?ïàƒ˜¦T"¿êF]ýŒ2S¿ãq
‰U~¸¿Ý:(e#ñ!¿î©"ÿ+Ý¿ïæítãìUNASNone?ۛ¹3Ьå?ÍÂø⟵±?â2#f©?ÍÂø⟵±?âWQm.ß?ÒÿƱQC;?ÛQ]%Û¢D?ÒÿƱQC;?äÀ.Ý̺?·KÂÒ8*?ÖÇ¢Df?·KÂÒ8)?ã¶4ácÓ?³ú³ˆ`±¡?ؓ–=9þ\?³ú³ˆ`±¡4FGL J1819.0-1203?îCÐÒ3`Á?ùé5¹qÀ9h™YùÕÀ:"Š.‹@ÖÿU¶ú@)ú}	@?ÒÐÏ:æ/õ?ŁÛw_‡û?öýŒ£ ?ûe¦MC?ïÐN+Ý¿éx¦¿òÉ·¿è ˜'[Ýv¿éþ_
¿âˊw½¦¿¿ïûï< UNASNone?êñ_`\ˆã?Ã|/ѧ?Ä:'~Üv?Ã|/ѧ?涺H€ðm?Óеjãš?Ғ‹nþ'?Óеjãš?äÃ-Ú*ÆÍ?¶¬_Ðsû6?Öy¤Kªre?¶¬_Ðsû5?átˆ'ç7?¼e¢ýòm?Ýáîú1'?¼e¢ýòn4FGL J1819.3-0935¿ÔLòeSú@>°YÏ/À9n*†¼GDÀ:Ç'*ç4W@áꛔÆv@‰1‡aˆ±?жšÙ4º?Òiëáºð@±îúôþD?÷L³è$l?ïÿ••_x¿±úfch¿êñ´âg¿é¿ü¿ç׏³•¿ïÿ!é^ÓËUNASNone?ãN†Õèá?Í热–û?ÙcÐòT.<?Í热–û?Ìý[7`u]?ÍȪĉ]>?èÀ©2'â¨?ÍȪĉ]=?Û¼ž%åH?¹IJÆd'J?â!°í
[ö?¹IJÆd'K?»´‡K9¢?¢ê´	¯Ö?ì‰oŸøÌ?¢ê´	¯Ö4FGL J1819.4-1102?éÿ)N
"?ÿ_ì»"À9¬m&SQÀ:žÄüô²Å@HÛìû@~@RiÄ¿¸?àôC3[w?ඥxÊìù@ûç¢;(Ë@£;Xñ‰¿ïðÞú̺X?ï7ÐQ¿Ø'k>gnÏ¿ê'ÂIÇI¿í}tՔòk¿é"[å$xUNASNone?‰Q{•ll?ša¼êÆûˆ?ªOƒ?ša¼êÆû‰?©àx†fÞî?·Õè–Ð?îaøw™'?·Õè–Ð?Ätµ<߁Ç?«'£yšP&?êâÒ°ÈŽ?«'£yšP%?­Æ§¨? ÁOº—-Î?î.ãžFõ…? ÁOº—-Ï4FGL J1819.9-1300?ß9Š/9vˆ?íØ⟜èÙÀ8Ä,5èðÀ:BÁE°
@ÎÍ&8ú@×6žË2?Óí¶Üöe¢?Ѽ)çZ?ÿÄô@¯¹?ùŒ˜êS¿ê÷–¤ò"0?ÝîÅû¢MG¿ëõÄÝëB¿ê¯:J~©S¿àvÎ}üÛ¿ê¬çŸaÑUNASNone?ÚÊcX5Ÿb?Õ-ôJr]?âšÎSå0P?Õ-ôJr]?¼´9õÖÑ?Ço—
7Æ?ìi|øÁE&?Ço—
7Å?Õ߸ à?¸P§x Í?åx£ïð?¸P§x Í?¼¯8d»¾£?±ú"ëøå¹?ìjóhˆ+?±ú"ëøå¹4FGL J1819.9-2926¿ïÔ#EÔÀSÀñˉ֮À:ª3DÐêÀ;Óà{Ö:@˜p¤ý[@¦k|OÜ·?ÅÊE
K3?Õ[Á<ëÙ@g/3Ê1è@AyúíÇn?ìvµ~|‡»¿Ð—¿ú¬Y¿å7ÌÎû¿áFJÂpþE¿î^%"ôÆç¿ïÿÿ^ðP`UNASNone?ä:'CW?ÈÝ! ӛ?×ÊÛyQÈ?ÈÝ! ӛ?êÒq>»þ?ËÀbkÄ	¤?Ķ;í?ËÀbkÄ	£?ÞµEE¸üÐ?»/LeM¢y?à¥]]#˜?»/LeM¢y?ècG'q?­W½[yU}?Îrãb;¯¿?­W½[yU~4FGL J1819.9-1530¿ïȼjðJ´¿ÐWÁ•aüÀ9gLÖÀ;#ƒ×u.@FÞá¢G@í>" 
Q?̾­º¸Î?ïÿîbHÊt@Ôb^™éK?õ'{è-Ñ?å³ý">5Æ?ÝdZÝò%?Ѭ{ÃŽ¿èx²>@ÿîR¡)°Ó¿é©ÃGèÌÞUNASNone3FGL J1820.3-1529c?h8ÊLÇ?¡ˆ×ÔêFú?ïççÇ5â³?¡ˆ×ÔêFú?|}Âç8m?ƒÑqÓ¥Ý?ïÇz1я?ƒÑqÓ¥Ý?¥³8áo?™Å÷šj{?î¤Ì~é?™Å÷šjx?	Žz"JÎw>ÿ£¶^}_í?ïÿ™Æ®Õ>ÿ£¶^}_í4FGL J1820.3-2646?êå¯3ÌâÀƒëaãIçÀ:-îÉp!À;uñÀ¢@Óaš#Ø!@¢¢dCvw?ÔLÄô;Q?㥾/ûñ@©Ô•*™?þ"¡Û1"x?ïý
<(¥;¿Öy7¤\U¿éâL@Jrë¿êÞ́®Á¿ïá¤_Æ95¿éäL —©UNASNone?Ýýæmý'?Ðʬä
¿h?áÉ7?Ðʬä
¿h?Û5tL‹þ±?Õq¸ü»?âeEÙº§?Õq¸ü»?×+RŸ)\?¹:"	A|E?äj}Ö°kR?¹:"	A|E?¤ë»'»0á?Œ˜j"'Ýû?î±DM"Lò?Œ˜j"'Ýû4FGL J1820.7-3217?ç}4ÝuÀ wB™ØƒºÀ:"Ô+|À<WÔUWJ@$‹Å¦Ê?þÖË8x'?Ñð\žçaN?çmjW@KU}
Ú?ÿ§‡ Q»?î[õÊd?î±ã<zÛ¿ÆQ$ŠÎÑ¿àGóÿÁ–¹¿ìUŠÁ9›­¿â]ŸˆUNASNone3FGL J1820.4-3217?¥a'%Îú?¨%¯iMŠ¾?î¯y퍣?¨%¯iMŠ¾?±›Ÿ³¨ç ?ºW3×zU?í̌	Šã?ºW3×zU?¸Éž'€¤"?£š‹šny¯?ìæÌ;ën?£š‹šny®?°ŠÚ·¾t´?—þÍöòx?í1i?—þÍöòx4FGL J1821.5-2531?ê-a‰x À&,ýxÀ:úmïǤÀ;c\Äüô³@àû­àÎ@4@^"àÍ?Ìj(è¬|J?ÉÙ¢Ò1f@8ݗl@íÚ£úñx?îÿü¿¿Ó½°d·9¾¿ê$'ýuE¿ßL‰°îIõ¿ìòSš¿ïÿ7ûþéUNASNone?äQ¢·›ÍÕ?ˈpúSÿ?×\ºÈdW?ˈpúSÿ?êíWï­÷X?ʃä›E#±?ÄJ AH"¡?ʃä›E#±?ã"©m?ºÓüI"ƒ{?Ø×÷Ä­Å'?ºÓüI"ƒ{?åÔëB?³Ñ^wõO	?ÔV)z"Ðí?³Ñ^wõO	4FGL J1821.6+6636¿å4°k=ZÏ@;ª% Jù#À;(o`àëhÀ<Öö¾7ޔ@ è¬Û•½l?ühžŸ'×Þ?ÃÈÃRЇl?¯©¢?g¹?íýú1@	ĺËÃbk¿ìÂmÎ9´W¿ïÿúâô?ïÿíUÙPi¿åØQÀ'ô¿»OÐ^
¿¿à^¨A}"ëUNASNone3FGL J1821.9+6636?ïÿ¯ì¢ÉU?©''ãШ?×Mªï#?©''ãÑR?ïþn¥zc¥?Cÿ>Ã4|¯?)¨Yųz?Cÿ>Ã4|¨?ïñ³{7‹?f$¬i'WÆ?\™	ãé©?f$¬i'WÂ?ïþü@ƒ¾i?ʯ›U®"? ;÷ÄjÉ?ʯ›U®Å4FGL J1822.0-3146?Ì6¨Ëš!À ySyú—áÀ:•¨þ'j÷À;ã)þK@ႁOù@4Ÿå
5s?ÊoEFl?§¿^5{ž?⦓}æO@>—…BI§¿Ú
ý‹["?ïþô1•¤B¿è@C=¿Ý'œdÐK¿ëëÌ!+HÙ¿y¹!/‹ÅUNASNone?ï|t4
?…Iz_??~ñy~]r?…Iz_>?ï㖱LRË?†­a+…'‹?liN³­5ž?†­a+…'Œ?í¨ÊëÁ‹?¢#Wú°Ù?²¹¨¡÷›ª?¢#Wú°Ù?ïLÆÃOBü?‡gw/±?–g'– y?‡gw/¯4FGL J1822.6-2502?ÙR•‰Ð±À½Û˜A«À:q7öçRŠÀ;…yB=K@ÞM¨ªY@´ì O*à?ÕÚ/¡XTÖ?à"Ìô9ù@Xæj,Å@°
©¶È¿â!֝l¿æð+¬V4À¿Üɀ2Wk¿æ®°:Ê¿ïÿϞcWé?äæ»@2uUNASNone?Üá¨7êÙ?Ðù78ñÚ?á+úd
"?Ðù78ñÜ?å6Œ"=Ü3?Ô  ì·\3?Ւæ÷"G™?Ô  ì·\3?Ցeÿd…?¿3®‹£Zò?å7Mqͼ?¿3®‹£Zñ?Û<쐸?¿"`ªØ¯ ?â}ቷÿ¤?¿"`ªØ¯ 4FGL J1822.8-1118?æùóZøJ?ñ&Y0þÀ8çíåÀ:TK8ãv\@±Õ>ì¥@ÃJ‡ãŽ°?Æ~Jž3Ý'?ÂƇÕvê?ý¹|X@2ö?ÿì0àr›ÿ?åxÿnw­¿äƒÛÂ3¿è%Ò݈ó¿å'úhçJ'¿íTvyÙಿïóܦ^£úUNASNone?¹…@ÚýT?Â|sh†Ž?ìÏWä \v?Â|sh†Ž?Üs;JÚnP?Ôwºï<'?áÆbZ'È×?Ôwºï<'?Þ	Z[µ?»çxyóô{?àûRÒ%rþ?»çxyóô{?Ôé
Mé×?´N@TúŽi?å‹zÙx?´N@TúŽi4FGL J1822.9-4718?¢†:5$ÖÀ.,ê(þ&À:cÞº5"À<6%ðT'R@þ 8¯žê@!%‰Õ?Ãÿۂr5¨?Ñ'ýž%ð@	N½ÅÈ̍@¡ØàVls?ëJ%󯏥¿Ý(¸ÛÔ&³¿ÞÊZâN¿+¿äÁtæX¿ïÿòɶ—׿ÉÅèª;}UNASNone3FGL J1823.2-4722?àI†Mw?ʞËž»2?ßmóeù?ʞËž»2?èܑ¨pPË?Î0·Î>?̍¹^>¼Ó?Î0·Î=?ÞX
‹%q?¹ÀáDM±£?àÓúºsíH?¹ÀáDM±£?é4\*º?©*þtm2?Ë.Wõ‡?©*þtm14FGL J1823.2+1209¿ïÆßë¢^@'eÿ'+¾ËÀ:Ó°QlÀ<ª¾
'*:@­B§šcC@œa½Š9ª?ҖÞ­?ïÿ¤%
ւ@D9ô"?ûfkâ|·¿ãÉ¢
cB¿âɹòÕu?Çñ½_œs¿éÒ¹
x)¿ïþdž;îÄ?¸xQJuoUNASNone?¹5ӗÍÌl?¸ø­Np\?ìÙEFs?¸ø­Np\?¦p¨â]J;?ºP–BÕ?î˜õqÚ+\?ºP–BÖ?÷ ìènæ?¬	…ÓGà?ë7ÄÅäF?¬	…ÓGà?}¡Iv±D?mžvÂê?ïĽmx?mžvÂê4FGL J1823.3-1340?ÓþˆIf!¿½kW½VÀ7d_4Bý¬À9Ðè±.á•@VIã£Ô@0k_Êjó?¬b¡œ»­?ÏWŠý@Áæ??öÍþîˆx?êÔ½‡	Ÿ?Ó¸GD7<'¿à¤¸F-
û¿ã!½êÜ­¿ê
Ä
áj¿í¼ã`7"VUNASNone3FGL J1823.2-1339?4e€`?0³"3m?ïýsOý4?0³"3m?i¶ŽÌ­o?r¨Á/1?ïæIq3Rì?r¨Á/1?Ÿw£™OÎ?—›™‰ex½?ï$Bã5'?—›™‰ex½?c'Èé|‹?f—c'~Ò?ïÿ\ãi¸´?f—c'~Ô4FGL J1823.8-3544?ïJGgzöÙÀ$³H+è¼À;!<ÝÖàLÀ<­‰;}…@³GC¸?ÿŒèæÞÆÊ?ÓÒ\Ä&5?å±	!ç±U@HŸž–Xœ@µy'=/?ëLѿкî?íVˆm!k‹¿Î-º"{*¿àò÷ÙÀÑ¿ïÿŒri©è?è»K€1ÈUNASNone?䚏%9$¸?ˊŸ…êø(?ÖÊᵍ¶'?ˊŸ…êø(?àBáâ{pŸ?Հדñ¯î?ßz<;	Ã?Հדñ¯î?Õ?ÅéÄ?½w"Ë ?å}àv?½w"Ë ?ãt`C%`?½ÿÃÛU~¯?Ù?Ãyµ??½ÿÃÛU~¯4FGL J1824.2+1231¿î;&KôèÈ@'Fd+ùƒÀ9ùžã…uöÀ;°öüK?™@²è @¬6|"ÏU?Å]b[¿ÄQ?Ȓ›ãö´þ?ýF©î@tÂâ¾%À¿ïÿ²'ž«Q?ïÿú Âî'¿é3¼$Þܚ¿çn¦`ýEæ¿ïõpŸÐ?s?î"úÎg׀UNASNone?ë´§-¨‹?Âø¿Ö4´î?Á-cI]Ó±?Âø¿Ö4´î?ê0â}%Ù?͆Ai6Ë¢?Ç<w'hœ?͆Ai6Ë¢?ãàՕLC-?½ö·zH4)?Ø>TÕgy¥?½ö·zH4(?ì|ô;2µ…?¬1iËc²?¼^&jSÓ?¬1iËc±4FGL J1824.2-0621?â9­"Vp@ÐD¡À›À9F¿'țæÀ;Òê šª;@ݕܠªZ?ú7#¸kì¸?¾‰/¿
l?ãaŸËŒÜ@!gÛ	¦qï@>Ašÿö¿îYÀGƒL?ïñs	â×Ñ?Ä+üŸã‹¿Ô×~×v¿èUæ¼b~¿ïÿÿ" 5•UNASNone3FGL J1824.3-0620?'ÜúÊû]?'ÕXžØ}3?ïo)¨%?'ÕXžØ}3?u''ć? 0Dùˆ?ïÔûÁ°vñ? 0Dùˆ?ÕžqÙ?·xÙ°^êÒ?åp0þG}?·xÙ°^êÒ?ZPz–é?LZKt-%?ïò×´øÁ?LZKt-%4FGL J1824.2-5427?à1qiÀ2Œ`Ëò²À:[ùæ
‹tÀ<‡²ù¼ïà@¤lŸ:˜W?ü~CÖ[?ŋ)ÿ­Ê©?Û9»n€'@Äq´xB1@ð¾'u³¶?îy;àÖÄó¿Î¬xCˆ–¿ Ó¢ s4w¿á™i=[U;¿ïêúêíID¿ïÿö$´ë/UNASNone3FGL J1824.2-5427?¬mÜ·$ª¢?«²Œ©?î9"4µV?«²Œ©?¾á|û©
µ?È"÷yÓæ?ì#Ð`ŠÞª?È"÷yÓæ?¡Új3'…Ô?"û"†™?îâY\Æ×£?"û"†™"?ËØÙ}Ý|É?±Æ‹žJ?é	É ˆ Î?±Æ‹žL4FGL J1824.7+2403¿ÌVñ8áÈs@0HÙºÀ:œÑ¦PaAÀ<\G4q÷"@Sûª°Ã?þh¤~Ïé¸?ÕH 'Áç?Ù¯}HÖ@‹ÔÝ<†™@a4-.6t¿ï§x_7H?åì¡~ji¿Ý¥a~õÿ¿ã'&"©x4¿ëȽhÖ®¿ïÿöÅĚÏUNASNone?셯­{Ç?¹8+g"Ì?»Ò'"'ÙÊ?¹8+g"Ì?멵x-(É?ƸÅãœl6?ÁY*K\Û?ƸÅãœl6?æ»|µD=?´-Ց,Äb?҉•Áw"?´-Ց,Äb?çœéQ¶ˆ¾?°z†v§ì?ÐÆ-\'îƒ?°z†v§ì4FGL J1825.9-3153¿¨îñãÛlÀ"ÄÞÁÁ×À:"×`¤…†À;¾k#d‰@'ZïÅZ@ù4ºð!?Ïh`fþ?Ò@âô,@QáŽû°æ?ü†WÕÔÞ>?ïœÈùµ½¿åX=˜çÿãó"Çz¿æ:´ÒD2¿ïû]èHS?~+VUNASNone?ë_m¾ Àœ?Á
.8X?'I|ý?Á
.8X?ä~SSaì?ӁËqQLi?×YYá<)?ӁËqQLi?á¶ÂËâÛÕ?·<Aù¥?ܒzh:HV?·<Aù¥?ÙÃܧ}"q?¼.ňÕ]?ã¬A6H?¼.ňÕ]4FGL J1825.9-5614?éùÔúñ%À2ì|ÇÑ»IÀ:tý£.mÒÀ<W¿Úv@"¹._cé@\á>iÈ?Çòfh?Àkj1L(?ðu'a¼³z?þ±Naaï´?ïþ'¸«­˜¿äé5¹pß¿å¨tþ¯ž¿éžƒ¾ôÚ¿à2Ô¿ëÉú?KÅPUNASNone?ï쥇–W?i{´N¼Þ?cZxþi¨ò?i{´N¼Û?ïc›~Èsÿ?§Ÿ0
Ùc¨?"Œ&ñ€+?§Ÿ0
Ùc©?ï‰Zdq?"°ªõS¤?ç®Ô³qû?"°ªõS£?î"v˜3?'5钄ü­?¦¾¿¨–|Ï?'5钄ü®4FGL J1826.2-2830¿qm¬hüèÀXpƒڑÀ:zyöf#KÀ;åµWeA£@á]'£]@\¢}méè?ѯä^¹É»?ávU⊤3@«4<Ëb?ó|¥³Û?ï";ÞþR¬¿Ð»ÙÊâ¿é¦î¡ˆÑJ¿âTÿ5Õ¥¿ïÿþ½à ¿?ïÿÞr¾"UNASNone?Û~ÎâOý®?Ðó_m©?â@˜ŽØ)?Ðó_m©?Պ€OÐäþ?Õ hܹ£?å:¿Ø€?Õ hܹ£?Ôæ5›ۘ?¸¦˜õ±Ç?åŒå2r4?¸¦˜õ±Ç?ªônLÍ3?è¦?îP¾¹3-?è§4FGL J1826.5-1202c?ëN9
!pV¿­Í¶<ù–ÁÀ7þ)›Ú¼zÀ9îõì@ß·Ú@¹Æ_ËA²?È
Áúá³?Û«;³´M@ϱÀo?ûFîK¢•Â?焓xhҿՔÌÀ¸ln¿æwóÂî¿ìNwÇ·º¿ïÿþÐñ?íì|*	üUNASNone4?ނnÂÞ;+?ÛS0×3?à¾Èžâj?ÛS0×3?ÃÏ5#ËÜ?Í뤿4H?ë2·
?J?Í뤿4H?¹Ô×´õx?©ñŠ 3"?ìÅe	a_1?©ñŠ 3"?jCÂùyS?_óÏKGç·?ï值=‡?_óÏKGç·4FGL J1827.2+4303¿Þô¥>Ì"@6RÿŸ‡ð$À;$;ž;¿ÊÀ< j0'|@áH—žl½@aÙ¿#–Þ?Ñ
#hú?ÇTÒª²E¸?ôu"‡!œ?û[Õ@Ž»o?ãìá•0Ô¿êi‡]æJ¿Ç9`¿Û/dý/Á¿ì=#vý_¿ïÿŽ@)çUNASNone?Ï<Û°?‰ŠžnÒÚ?ŠPÌ0Éõ?‰ŠžnÒÚ?ïT
­2?±Ã0[ 
?~þJYË?±Ã0[ 
?îA7æÔ?Aÿï6+?«ìŽážÂ¾?Aÿï6+?íl{ó*Rd?—Ì÷(…í'?´œ f­lã?—Ì÷(…í4FGL J1827.5+1141¿ï߹ʣþ@%ô‡ü¹$À9ȄÚ`3À;÷é"mé@@ö¥8^@+¢õÚ?¼±4u¶?ÖÒóW{@v!`¢Ø@Š¥ÜÈîF?ïøTÛ#§¥¿Ø*¬¼aË¿Ü¿+Žúg¿áÑýžPãr¿íê¬"¢º¿ïÿ¶>@£UNASNone3FGL J1827.7+1141?—k "¡¥U?—™ÌʆL?ïD¢ûÚòÕ?—™ÌʆL?·~ñ…nJ?ÆÁòB
¦Ò?í.ÏR6?ÆÁòB
¦Ò?©ÄɄ+? µ9ÿIí?îc¾ŽÓg¼? µ9ÿIî?Èwo'3?¦n{Kñ?éÿâ$zô?¦n{Kñ4FGL J1828.1-1312?î'(L"X¿íƒîÓTPÀ7酵·'À9s7+æ7Ø@"ž >¤V@mPes!?É!Þ!3ˆ?Ðå%ßÀX?þxøŠ.Ã?úaÂgÄ
¿ápÈà.(‡¿êé/~¿Ä¿åÝÐ?ÈíÅ¿é'9@=‡Ë¿íçÀn¹¿ïÿîbHÊtUNASNone?â<¿ïû"…?Ò±2eOŸ?ۆ€ Øø?Ò±2eOŸ?×îP¯+ö]?Õ$rà'M?äרjÒ?Õ$rà'M?Ö|"ƒ}#?µ­sã—Ê?äòÁ½¾Ao?µ­sã—Ê?©ÿ»a¸Ë? œ'Híð¡?î`Nät? œ'Híð¡4FGL J1828.2-3252?ⓄMŒ5³À#˶ˆ½©CÀ;)mã2iàÀ<¬ÝpÜ@ûàÖÄó:?ú®!ÛòÚ?ÕØá-,?å'Á)h¯@
`9[k`¡@Kº5›mY¿ïߕÇ}³?ïÿ;F',¿ÊŒbN~¾¿×<(¿íwi¢ò‰¿Óã~T™µHUNASNone?îmWY»ÞB?§Z±+à?©*ŠdBï?§Z±+à?îoÖ×âÃ?¼BÀí-d;?©'AÓÑ?¼BÀí-d;?é5½AÁ?´6ÍÎ ?
?Ë+Ÿù
øú?´6ÍÎ ?
?ìµ®Õ6<ø?¥5§T_mÔ?ºR‰VND?¥5§T_mÔ4FGL J1829.6-2545?Ô9roöÈÀ"`št‹À:unF.¸zÀ<HåC¼s@ÓÜäòÞ@OC427?Ó-&ÿž0W?ïþ
hø@!G'R?ìђ&ç( ?m¿Ýß<;±'¿ád¢A¿îqkGv·¿ïúYbqå ?ïå«@
11UNASNone?ãŽgíÿ0§?Ôëí´gó?Øã0$ž²?Ôëí´gó?ÉPÀx™Ã?ÒøiüKEÀ?é«ùáُ?ÒøiüKEÀ?Ǿ78>Ú%?­žÎÆPã?êr1ðIw?­žÎÆPã	?T–&Cã´?M¶†ãO´?ïõ´ìú^?M¶†ãOµ4FGL J1829.6-4310?îíֆ>À-Ǽ"ŽÀ;>@ÈG,À<Ñý¾Ý @zú*O	@Ôj»_¼ÿ?ÔãÌ"'áÇ?ëÊÝßCÈ@	œ?,eº?ÿSƒþ&áì?ë©È»ÆL¿ã‹¯Rhƒ¿Ä¼=Þ\í¿èwsÔãòƒ¿ïÿþÞ÷¿ìÌòÂ)ۜUNASNone?ëâcýp?ÂC<ià|'?Øvp
?‹?ÂC<ià|'?á;aZñô?ÕÁXÚ!×Ï?݉=JÑ?ÕÁXÚ!×Ï?ærÄ$*¦?·ûûcO·r?Ów·Çª´?·ûûcO·r?Ë
MF*ß?²Q {Mf?é<¬®|õH?²Q {Mf4FGL J1830.0-1515c¿ÔÁ,íôúÀc÷¦•*ŸÀ:IVH1ŒÀ;Û¸øÚr@"k³bmˆo?ÿXß_vˆ?Ÿˆ¨}®-¿¸;øÿ…±°?ñ>Õ'å!@Þø4Y£à¿âž%"ôÆç?î{P}ñÈZ¿é|í'hr°¿àòG°˜¹ ¿ÔɎÿ·°±¿àz 9påUNASNone"?ïêڗHŒ ?eßÖ2'ݙ?e%h·saB?eßÖ2'ݕ?ïÈ¢Œw?¦@°˜[ˆ9?{À.À9ÄÎ?¦@°˜[ˆ9?ï'>ð|?–fÏWÕß?Ÿ.[!ðw?–fÏWÕÝ?ï
;`›ƒ?…Ï~«PCó?X"쏏?…Ï~«PCò4FGL J1830.1-0212c¿ï èVÕ@
×õfI
À9?|–S"üÀ:́I@»²@Uñ3^|7@]gº#}?Êu¶e':Ø?áPVY¨èÂ@¥Õo2½Â?üLH=0?îˆ@
²
ª¿°†òÍèU¿¿äF­czù›¿é³©Xb˜¿íÙä"rÁ?ÐyM>!MØUNASNone3FGL J1829.9-0203c,?u27:¶Úò?yQk;Ÿl?ï՛'Š'J?yQk;Ÿl?£öyĶ!è?¸CՄž?îÀ˜c´â?¸CՄž?¥±ZðƳ+?"S¶þB‡{?î¤êPó"Í?"S¶þB‡y?|Þ¢Ÿ"¦?h²›Ó'•X?ïÆBºÀÖ´?h²›Ó'•X4FGL J1830.1-1440?Èe*_óg0ÀWµäRûPÀ:%ý®(`À;Y.Œ…¡@!a÷q'á@èû"°ý?®_+‰›Ÿ®¿¹%ya?ñK&õ7O"@)$衦?îçYޘ§¿â{ê'Ù±¸¿àÒZu—[Ò¿âðóˆ"xÑ¿åIׄ¶³†¿Ð?"$ghoUNASNone?ï³Ø~®È?c'-.^?ƒ	àTMý³?c'-.[?ïfÄx‰E?±€ÖdO›¬?"'pî×P?±€ÖdO›«?îöQ±}%?•Tæ§Þus? šäîè-¹?•Tæ§Þut?î€çÌ
´?›6"ГU¤?®Gñƒ?T»?›6"ГU¤4FGL J1830.3-1601¿ê{½¿™Ê}À¥Ûüëx‰À;;?´JõÈÀ<«Ü'<®@&~Ç!' ÿ?ò(IDíoÛ?Ôπ0fû?ÂÏôŸy­k?æÒÎn|@Š'‰)ßÍ¿Ì[/ürù¿ïúÙ_­9µ?ïò×ùP¹V¿ë¤šéû±½?åg*¡iFÁ?ÎUå]gUNASNone?ïóUëÁËî? .úFÕ5?YT(|h$ž? .úFÕ6?ïÚ͙Í5q?£­sç?r™3eGß?£­sç?ïS³VãØC?''PàR?•‰•#"÷¶?''PàS?ïìô¶C$[?nâ
µ*ü?cI¼Û¤Ã?nâ
µ*ü4FGL J1830.7-1634¿ï«wœ—ÖªÀK~ƒ"×À8û6)‡¸ÇÀ;&‡¹E @P`@@̘å>³š?¸uË°4?ÍEɸÆ/¥@çtü+_)@Gx¶Ë¿Ä˜mŠ#!¿á*ÀH&¿ß'7<Ø"–¿ã‡ÄŸ×¡<¿é­Ìâh'¿ðUNASNone3FGL J1830.7-1630?Ó%ÊuÞ…?Ç4žw"?æmÅñ¾?Ç4žw"?ätçñ´†¾?Ó#ýyG%Ï?×0–ò…?Ó#ýyG%Ï?ØÑ›©d?º3é)jÿ÷?ã—@2|«N?º3é)jÿö?á]"Â;X?±RƤtI?ÝDÖ{á‰P?±RƤtI4FGL J1830.7-3219¿½ÁJàƒŒÀ$K-
$F0À:M)¹6íÓÀ;ï>FŒ¬K@
ovZzJ@òǝ¸ã?̱¬µÖB?КtŒB@K/©:÷M@]i·?ìŽPrß?ïùâå=¿å>f˜¿åOÍ2MZ&¿ë)˜JA¿ï…õåÊËUNASNone?íñ2
NP8?­qW*´&ö?°vo­~=?­qW*´&ö?î™K!M?À…'Õg—?®Vn{Më1?À…'Õg—?éJÈÉl?¯ÞöÜC²??ÊÔÜÛ³ÒQ?¯ÞöÜC²??ëà×ÑE=þ?¦ÙwøA?¿?À| ºë?¦ÙwøA?¾4FGL J1830.8-3132¿ç×#/‹d†À#aE•6À:>üGä› À<f°b2úÿ@ø$ EŲ?ýÖjÛ@-?Ãöó<?áwT€	û@0tBÇû­?÷ŒÈ¨zÝí?íÇh¿‡¿Úÿ'}ž;?Ç؎÷Õ:¿â,Æœ/¿ëº5¤¿ïý¾1)UNASNone3FGL J1830.8-3136?Û¦ò¤Ô~?®¶ýUò?ïy"ÈjÙ\?®¶ýUò?–M÷­Ù>?¤œ÷Xa?ïOB'6?¤œ÷Xa?™™ÜòÆz?Á³‰ß?ï37¹iÌ?Á³‰ß?Š^¡J,ÇW?vÓôÐ#7w?z×Lã?vÓôÐ#7x4FGL J1831.1-6503¿ïíȉ½;ŒÀ6YTdÜ"«À:NRå€!ùÀ<‹Å£ãŸw@$Á'|D?ýŒMryš?Àúpßf,…?ÛRº·÷R²@RîcŠ	?üܼŸ‰?~@ÈG,¿•sG R›X¿Óðe£ráI¿ã˜a‹5S¿íçJýTT¿ïþ®û*®UNASNone3FGL J1831.6-6503?'*¾³¯"?'+ƒ^,Aá?ï·Wµ1B?'+ƒ^,Aá?XÒúϦ?ªJa¤Ø¨£?ï=9h)ƒ?ªJa¤Ø¨£?–°ÙèEÇ?Š:^)ª?ïJ¡0½Ñ?Š:^)ª?¢ß	ƒ®D(?‹Çz•á,å?îÒgŽ?‹Çz•á,å4FGL J1831.2+0202?à3eì¿)Ã@¬óý">6À9ž;1.v5À;¡]³9@sŸ4
N@7ÜËè¡?Ê]u&Ê;?º;²!""?ïwLg·Ÿ@Ñ#rJö¿ÁŒˆy‹²%¿Ù'k\ÅRÛ¿ëÝQŸ"ë¿âKu°†E¿ä0#̎¿ì$P±*UNASNone?íœ`Ngk?±‰Cå]è?³ýŒÄ§Ó?±‰Cå]è?îèÕª0\"?µºÎƨ"È?¡r¥\ú6Ö?µºÎƨ"Ç?ëQ¸£&.þ?¯3&PÙ·Ð?¹sgD
?¯3&PÙ·Ð?ï.ü9Dæ?ƒ™;ˆ=
ü?š x×c>;?ƒ™;ˆ=
ü4FGL J1831.6-0223c¿îÛya à…@
orÖٖÀ8® HtäÀ:b4"F{å@~og–è@ñm*¥Åø?ÆèÐ#ˆã?ϏŠâq¤³@?òÿf}
?ù~‹=á7?ïh
?®–¬?ã"Ág	¿ã^PþJHN¿ævéki¦¿ê±ôÆ/¿ï÷™^á6çUNASNone3FGL J1831.7-0230 ?˜ùÅX4eJ?žk£Pü?ï81Õ>\Õ?žk£Pü? tù.ûl?±òîÝd§…?îø°mI??±òîÝd§…?ÃeÅÞ•y?­þ¾R¤"?ë&ŽˆyZ¢?­þ¾R¤"?SÝçÈAD?€Àœ}4Ó?ï}aÁ½ö?€Àœ}4Ó4FGL J1832.4-0152c¿åý*aí½@
û–C£Ã¿À9*螺jÊÀ:ŸFŸ@èˆòWuÞ@ŽY½
·ê?Å};‡õ'?´Œ5'î²P?ñ³WN›o?í¹ž"!­?ïŸÈ‡Ã®@¿ã³Ú°¿åÓZ'És¿êYÙUm¿ØCÑ(l0¿îûž ç×UNASNone<?íS›È­h?¾©Qu7?µg›!º"¼?¾©Qu7?â ÎÒÅ?ÖXɊ¶?Ú¾b[Ïæx?ÖXɊ¶?荋½¬Õå?·¬J'YI?ÍÉÑ	L¨g?·¬J'YG?ÑüOAéQ‹?»Þ9¶L?çØ_W:?»Þ9¶L4FGL J1834.2-0827c¿»ß}¾É¿²\›ao܇À88+"Ù@yÀ9­¢uá-­@'£Ýë-@D@yJ?È%µœ.ŸP?ãÖ³ «Ü'@[WG9?ô'qº,Œ%¿¸ºË,Ž©?áÌ•¶¿áP‡×Ð6¿í7åžTê¿èœåžªÐy¿ïõ'àhUNASNone0?pÀ¡°B&×?§,º"ȉ`?ïÞ~¼Ÿ{²?§,º"ȉa?ˆÖVŒÉ?¢YÊíÔº?ïŸè¦¥ÉÍ?¢YÊíÔº?¸	Ûè#?§Ð—ÞÕã?ìýþĂûœ?§Ð—ÞÕã?"
À¶÷Qž?èE¹J˜?ïþßSô‹?èE¹J˜4FGL J1834.3+0613?Úöĺ·J@‰¼Ö_À:/ÞM'ÐÿÀ;èPÕ©³@,Eü
­@lKÅÑ0	?Ç·v¤L%?Ûê-/ãó@
Ew{a .?ù™²
ԚL¿äIq-iŖ¿ã»àÑn¿ßù;.ª¿â=@26ý¿ïúá¸\?Ôùr²¥ZUNASNone?·¸æOH»â?¶'­´—r¤?íã6èƒ?¶'­´—r¤?Ð:9ýY?шªÓƒÉ?çâãSrõ?шªÓƒÉ?ȶ;bÓó)?³_o0¢7?éÒq'K5?³_o0¢8?Æu?'?­#3z×ô?ê{¢¹0:?­#3z×ô4FGL J1834.7-0724c?脈 Tt>?Óñ(̧ãßÀ8Ní·þßoÀ9ógÁLf@CÏ*J+r@7õbLM?Æ('Á—å?Ýdéc±UM@_Ɨ(¦@I¯¡mÎ?ÖÔÀdïn¿Üœž^€>¿áWàÌV¿êÁ+Xô¿éûÔÂd"þ¿ïÿß~€8 UNASNone0?ËÒQ†ž=?áJl5?ï¡msË?áJl5?'øm×1?§XAb7}H?ïh?"—IF?§XAb7}G?žþà0BV?"2PNiÜÐ?ïþ}íP?"2PNiÜÑ?iÔďD™å?YP×Û^<L?ïæ+;p»f?YP×Û^<L4FGL J1834.9-0800?×{‡M÷ƒ}¿‹ò7jzr7À8²ò03¤À9§†P¹Œ@diÁºŸú@ÿ³Ä¾
'?ÃʀÂ2??Ú)åè
@XÁTɅð?úS—™åô?ïtôhó¡¿Üá‡ÚTtÌ¿å÷aËÌó¿é¤cOοïýv:ÂÊ¿ïñ`[_wUNASNone?ÕÏ`Ùù?Úã(¥¤$ø?åOö"w?Úã(¥¤$ø?ˆŽ'ß[?"k'ž‰0?Çñ´ƒ?"k'ž‰0?£Xƒ›lü?—Nóü÷O?îÊwΖI1?—Nóü÷O?3^`¤àFƒ?#TMh-nÍ?ïý"3ëcø?#TMh-nÍ4FGL J1834.9-2819?눣‡|ÏÀ"m‹`ñ²_À9ß)ã(XåÀ;¡?
×ÊW@A­RÞõ@õ†"X?ƃX$.]‹?Ì¿$³h£@©/¤2yÐ@jTXœÏ.?ï([žŒG¡¿äV¢¤W¿èû$Ų&¿ä¦^ê–¿ïþ×@Än?âÇÍSÛIgUNASNone?ìöìýd'?»ë¹ÉµUW?¸H˜ßÃo?»ë¹ÉµUW?ìÎ㙊Ø?ÄS<¦QÞ£?¹ˆã3©<?ÄS<¦QÞ£?éü€½¶Ü2?±Ð)}\??È
ý	$6?±Ð)}\??ì°ì;Ù¡Ç?¤cg‰¼?ºxž!2ñÆ?¤cg‰¼4FGL J1835.1-0517?Õ}5‹åß??óÄÀ:9tãë¸À;àæ½2%@¡ŸËŒÜ@N$PAa?ÔØèd?ïö?!}ÿ	@я1a@[î\>šE¿îäÍ_ê2?ï}ì?õ(?ØCôáé¿w¿éÍî \+z¿ìTÙÁQïa¿ï‹6môOUNASNone?‰›q6=;? q<Œ(Y?';'? q<Œ(Z?'g>-+?ªVÊnVSU?ïotÆ—?ªVÊnVSU?ÁÔiØ›É?¬JûF?ëŠå‰ÿ™
?¬JûF?›FSß*?‰®ÄÉ°ä?ï%ÍgŒ?‰®ÄÉ°ä4FGL J1835.3-2439¿îaR:ÛtÀµK 'ßÀ9¿WeA£8À;]Û8 Z~@2۞ ç×@‹@š?Ä2·¸=Ÿ?®h²ñÚMi?êHQY•?ýŽücé4?ïñ"aÔ±H¿çMž§öT¿ër4€:M¿àõÓ÷cyL¿êm)™V}»¿ÛVÂd>UNASNone?îùW¯hC(?£KS|üÓ!? j…	{͉?£KS|üÓ!?îû-Z;îÚ?±8þݬ? M*\Ab?±8þݬ?ì·[žÌ??¥™ñrô¨f?ºE#	ü?¥™ñrô¨f?ì^_þßxi?£vJ±HÇ?½
	<®?£vJ±HÇ4FGL J1836.8-2354¿ëè×m,À"?ãDÞVÀ:BžHUÀ;¯ô"q<@
BTä2ð@ä¼B;
ó?Çè-%}$?Þç	úTÅT@*ܾ²W×@ôòÌæ£
?î)Xb—¥¿Ù¤›À»F"¿à]/…ÿ‰¿éÅ>=}d¿ïúȈšmÕ¿ïü™^
wRUNASNone3FGL J1837.3-2403?°P"1Üü?°;…
6?íõïnYÄ`?°;…
6?ÃŒãGŽ?ÄlÊD£ì?ë;Ç.€?ÄlÊD£ì?©¡ô~f?šŠ§þ*¹z?îeï¸9?šŠ§þ*¹w?ÃÛÞ-˜å}?£Ž_&¾Ù?ë	t™Æ¡?£Ž_&¾Ù4FGL J1836.9+4439¿Ûå Ë_õÃ@5!S‰Ò|À;
»DåÀ<Ì&Tþ_@ ìw‹§¾u?ý7†ª×¯?ÒQ/|}?Í|õžþ'?ö5…£BÈ@AÊ¢ûíø?ïÿn?x»Ô¿ïÿ"~LŒ ?ïó˧nn¿âº‰ yÞ¿ß:i]f¸q¿ÖÏo~èé8UNASNone?ïü!ëÌ?B¹¯ÖãÅ??þð¡Ÿá?B¹¯ÖãÀ?ïùÈ¢'#?eõ­ã?HÝwÁ·xß?eõ­ã?@fõ7?Šw)éþg+?oæB²m?Šw)éþg-?ï¿£çî¸È?rÛ´ yÏ?€QÎ
?rÛ´ yÎ4FGL J1837.9-0620?ê,L>Ùª_?¸Þm^'RªÀ8œá8"œÀ9ÔQžXE@äq–ñº@…à1?Ím6d@y?Ò¹–å	Y›@Ùs¤<ŠË@#ûó+g¿éMóÉøÝ?Ùä¼Îa¿åvÿ:Þ"`¿Ö=9T¿ëÍ/(·Ä¿ä?©þk«UNASNone?¨õDÖ
ò?½GZš1P?îp«²Ÿÿ!?½GZš1P?ž$œÖ=ß?±%'Þª&?ïÛOÆ?±%'Þª&?ÂyÏ
©?«kUî\6C?ëa½Ì<•?«kUî\6C?´\sƒ4?§Ce¬÷)®?ítqœ>y?§Ce¬÷)®4FGL J1838.1-3352?ão4>ÉXÀ(f¨ü
,8À:·?Úáb†À<˜úà@*¬C•V@茊½^?ÔzD¿¢˜?×c0œ*¬@|íáðJ€@u+ùX?ïÿÏ"èbU¿êƒÙ©T!À¿ÛÆ\Õn¿æÈl뻥]¿çžôí}F}¿ïü¥'†·UNASNone?ïÒâC}7?}ø¤F#
¢?vŽÞ|AdÑ?}ø¤F#
¡?ï6¤·Ùv?«µN?ÏW?™<iÑH?«µN?ÏW?ëa†e¿CB?®>ëÖ>?Âyæiòù?®>ëÖ>?ísÌ."Œ?™"÷œw<E?´až‹cŸ?™"÷œw<E4FGL J1838.2+3223?'¿d§¡<y@0´£ø˜,²À::Å%8ž­À<Ñ%÷áN@°ZŒ¾iÞ@^P?³t6?Åòw×'É?Ðÿ ß‰@ºVwÜ?üºËÃbk¿áòýž%ðU¿Ñ	£ðÝM¿â͇<ŸÃ¿ê7‡UÊ6ð¿é5:ßÏÞпïÿöùŠpUNASNone?àAÙˊGw?É6DÃّ?ß|Lhëq?É6DÃّ?â`ð[@µ?ђÝu·>2?Û>I~•?ђÝu·>2?àü·T	?ºLóP+Â?ÞđWíè?ºLóP+Â?àBhÎÎÅ?²½%ڌ‡$?ß{.cØbw?²½%ڌ‡$4FGL J1838.4-0630c?ëΐ>ÀÊ¿¶5U"…XÀ8ÖòJ¶ÝÀ9ßL¤@!7væfPí@ÙÒmrÊ?âh°ºG?¶'à~ÀÃ?òÈ4L7æ÷@—IEbø?æí½¨l›4¿ë,$ˆþA¿â*Œ 	_пéÇô@.C_¿êf££׿©½ï¦ìhUNASNone8?Î!‰aI"?ÏY~/L5?èw»§­œ?ÏY~/L6?ç"Õ#€üu?ÕeÌò؟h?ѺU¸þ?ÕeÌò؟h?ޔMlÀWì?¾Ôø*•?àµÙIŸÔ?¾Ôø*•?ãÔ÷ûЊ?Öʶ?ÙèV^ì?Öʶ4FGL J1838.4-0545?פ¦Y=dô?Ïþçüþî³À8Pª<À9LWšÈÙ@#ì°	‡@1ó:ß¿?͖9'ÈÅ?Ù²…"êÔ@<¬Ñ"Âr?ôªm9>e?ƦÊYªì'¿ÓÁ*¡OÆ¿ä€þ "o¿ç¸ˆb½Þ¿îxIRYi(¿ïä$7í'UNASNone?ºo\ßÃà?²Œ¥'¿?ïBŒ€ñ?²Œ¥'À?"[Sâ÷?«Kø¡ÚSÿ?ï_m'õ`è?«Kø¡ÚT?£¸âwª†}?'xL²Ò?îÄq؅W˜?'xL²Ð?DËA%¢q¿?5Ž¡ïƒ!N?ïúÍ/¶—d?5Ž¡ïƒ!N4FGL J1838.5+3837¿ÂÔ
®'è
@2áô™=SÀ:µÌ÷"÷sÀ<[]À¥w@"?6¡§°@Æñ'9y?ņ¢Ücm¹?ƒd·î!
õ?¼öxýí@õýÁ¿Îeô{'r‰¿ë]BÑ5è¿ãù½@gÏ¿â?õž}.)¿ïý'ÞZ"¿ê;Ì^èãUNASNone3FGL J1838.1+3827?ïÔG4YA7?wh¥4I°W?uÜeÓ_d¾?wh¥4I°X?ïוV'çh? ž†£Ìlù?t5TìKä? ž†£Ìlù?ïz8ÉÊ^´?Š™\2"7q?¸æÆ´)~?Š™\2"7p?ïÖV¾Ðµ‡?b)ïìlÐ
?tÔ —¥<M?b)ïìlÐ4FGL J1838.7-0601?áL8¬®?°uÙöÖáyÀ8öþ	…»À9ýtšÜ¸@"Ž3ºí|E@ir¥9

?ÏufI
5
?µú¥D"?ðŠ"˜±<N@֛öEŒ¿Ý(âø2V¿ÀQ°â5"·?ͳb(¤9¿ß¼¤`œøÊ¿æ{ï?z¿á©ø!mUNASNone?ÜSÑ'y°?ÑÈ©	$?áÿÖlC'?ÑÈ©	$?è5" 4Ý?ÔeŽغ?Ï)¯‡,‰?ÔeŽØ»?áñÇDÙ?ÄN*ÖÚ¯?ÝÑèqvN?ÄN*ÖÚ¯?é|kà‰"^?¼VIy'O?ÊP}Ùî‡?¼VIy'P4FGL J1839.0-1502?èøŸÏÚÀ‡zA¾	À9–ä+Ž#À;4Á5¿Õ@Ÿ?´öÂ?@›:Æ¥k_?ÉCáè<ë?ÓKaþ!Ùo@ÊôW@eÜRÑ´?ïÿHë+\¥¿Ý2/'"š¿é(¯ Ä¿â7wÀÖÊR¿ï®+ALP'¿ïÿø]ˆòUNASNone?ëñûîœþ?"´$š?Ãð8EŒ?"´$™?êi?Ëy°+ás?ǃµú[³Ï?Ëy°+ás?âª0ø"?·Iη'E?ÛØ«žzø?·Iη'E?å'0"Ð-?±sÌ0[u!?Ôᱟº_¦?±sÌ0[u!4FGL J1840.4-1705¿ç±€x'ýÀ]^^Z(kÀ:NH;Øô"À;¸©Þ‹;2@ ‰iw½Ñ²@½D™?ÒYª–A ?Ì'—ÉŠÍú?üö¡ÍDÁÑ@xœHöi?ïíTa$X¿îL'\f2?Ùþb;^zà¿å°ý-½¨m¿ìêÛ@-¹?Ä=må™!UNASNone?ë˜bâˆÉï?»½/!e7^?ÁžtuÜØF?»½/!e7^?íõ,•ù¾W?"qõšþ?°V›P2
G?"qõšþ?æż›Â¡e?´ÝjB*b9?Òt†Èz½5?´ÝjB*b9?éDõ>D",?µc´	ÏÉÌ?Êì+í³P?µc´	ÏÉÌ4FGL J1840.4-1139¿èà½FšÅ"ÀlÀóz¶À:™[†8"À;ø÷§kê4@ËK;½›W@'Wɱh?͝Çüƒs½?ëkö}ö%@œ(²¦°Ù?þ8›7(‹:¿ïým´8Q?ïÿñ¢o+1?ÝKáÕÈt¿çW½@½µX¿í¬¾¿ÃÏοïµ{A¿½ñUNASNone?s/sX(ùì?{spd™ð?ïÙ¡O®?{spd™ñ?³5kø^˜?ÃdÚ´–ï?í™R€ô,þ?ÃdÚ´–ï?¶àô¨Ú¬?¤íÖèT?í#ájä¿+?¤íÖèR?pëV=yb‰?`SS?Ž/)?ïÞ)S…
;?`SS?Ž/)4FGL J1841.6+7113?ɺ­ºFT@:Z–=Ć­À;tµcú{\À<ö«Yµ}ü@ ךÊF4Ã?ÿ׉¤Y=?Â$$wƒš)¿©CH ¢"F?ççf¬ƒ¨?ÿ¸Bi\ ¿ïìÎ?=­‹?ïüZžÜúl¿ç÷>Ælª¿ÊkÒ6?è¿à@H»ÊF¿æ&ÙRíÞUNASNone?ïû'cÙÙ?<sÐö?Aºp˜›¬}?<sÐÙ?ïù‹')zÕ?eî¯Í}?IÑ÷Z«Ý?eî¯Í}?ïíÛL°Z…?ik͛.Ã?b$³O¥{"?ik͛.·?ï¼÷¯²^O?pgQ ®%W?€ÂhlE?pgQ ®%W4FGL J1842.1+2737?ì[‹DLC@,+ææS†À:K½R†À<ˆd•y@Èü¶õJ?ü…Ö|?Ķ"‹ë[-?ä†ü^	öy@eê«%)@ÔCíë€l?æÀv蔩p¿¾z% x…ù¿©½XÚ©¿â§ÿ¸ÝW¿î͐ ôí'¿ïžÏÎß̄UNASNone3FGL J1842.2+2742?—­dÐË«o?´É#‰õ¦N?ïB"Ùy¢¤?´É#‰õ¦N?¬Ð'Á"SP?ß	˜'Ú?î2ýƒçºË?ß	˜'Ú?´rµ3JC3?¤ ²àˆõO?íq©Y–·š?¤ ²àˆõM?­Äoh`f?—q >?î#¹	yù˜?—q >4FGL J1842.2-0328¿ëïäŒÖÌ5?Ý:
b>8 À8hÞ4Ô#À9¨XŠÑ @Å÷ùñÉ@Òa¤_Æ9?õ¥ouÙ ñ?Émµ$ºt†@5%1?ûrEî¿ìxÄ'6N?íÿ*¿åc'K¯¿ì'<ðKW¿ä • ãû=¿ïÿÿÊPËUNASNone?â'2M4MŸ?Úm0|såÐ?Úݛe—dÁ?Úm0|såÐ?²ˆ$éJzš?Á"š7Èž?í®ûbÖ°­?Á"š7Èž?Ïé&`àÊá?¹ú
=R#?è¶gÇÍH?¹ú
=R#?²dB‹,¼I?·c!Xè£?í³w®šhw?·c!Xè£4FGL J1843.3-1242¿Ñ¢èF§WÀÿdIU´gÀ9Ñ{m^¨,À;pSÒ+í@Ž•¯4@£þwiÄ?Ì¨¯â?ÒåAbËÒ@'ö¿ž(@#V/ŒŠ'?ï;Eñ{ؾ?î/¥>éIÛ¿á<DSìç¿å«LŸjéٿ퐩e¿wz¿âÜþ=ˆ ËUNASNone?×úUy8ª?ÈÚ)ìã
a?ä}'ÕCc«?ÈÚ)ìã
a?ç÷-§QZ?ÒM'¨N?Ф°ß]J?ÒM'¨N?Þ~]J»ìM?¸"(ŽÕ[´?àÀÑZ¢	Ù?¸"(ŽÕ[´?â×ëÔÑø?·Ç˜"'Rë?ÚP(V\Í?·Ç˜"'Rë4FGL J1843.7-0326¿èÕÉÏpô?¹hšY³À8/r&À9|_æ¤í@W­»åt@ºd<Àz¯?欂ªiËv?¾²pK˜?ûV'QúŸ?ð•˜/âè¿mÜ	‰IGû¿Í—Ðk½¾<¿äÉh^Ž*Ñ¿éªÃø贊¿íþVèD!˜?ÜõÇb)ÀÄUNASNone3FGL J1843.7-0322?ɄL¡žø?ÒǕÇ&]?éžìטxB?ÒǕÇ&]?ÖÛA™r'œ?ÕÇüÄ8S'?ä'_3F¾²?ÕÇüÄ8S'?Ò
¿‹NŸ?¾
eƒa æ?æù :X°|?¾
eƒa ç?§dÌe·3? €s·þ–Š?9¤¼? €s·þ–Š4FGL J1844.7-2110?édg
¸öÀ +éȆ/À:Wꢠ©À;³§¬_o@W欜֐@Ov¼Ï)?ÊY&âÂØW?ÌÒ÷_Ÿù?ÿ'zH›zD@0‹1vðw¿×7¡2À?ïû@>Æå¿ç¦âøˆ<z¿â¯Dü‰Rú¿êàx`cíæ¿ï÷#b…±/UNASNone?èI
1y.R?ÅÅ»©>Ç×?ÎÛË:Fµ?ÅÅ»©>Ç×?îâ†:¼ì)?³ÄÔÿ¹IR?¡×œT1=q?³ÄÔÿ¹IR?çP¹A0"Ù?¹BB˜Û»½?Ñ^}žöN?¹BB˜Û»½?ía]߃վ? ¾²˜Pp?´õáR
? ¾²˜Pp4FGL J1844.8-0957¿ÏIµ¼¬mÀ‡«¨À9€_7ûÿÀ;Íì‡}7@Á¡w‰yf@Ö$o…Ê?ÌY{ÜÅ=a?Ôn›¿
Çi@tòñ#Ä*@¦Ý>ßå?ïæÍ)Á¿ÞôC~"ë7¿ácÍ.ò\¿éÐÚB×%¿ã#¡?€H¿ïü¯ž=Ã/UNASNone?å†Ú¸i]'?ÊoDݒØ\?ÔòJ-Dû?ÊoDݒØ]?èI³	ö?Ð*öHËÓ?Ϗ'Ù3Ø'?Ð*öHËÒ?àvÆ=8½ç?º	ɁI ?ßs…Ž"0?º	ɁI!?áEù
&)?µD"ìw?Ýt
å³­×?µD"ìw4FGL J1845.0+0159¿êÝТ¦ëË@¡®ÁIÀ:Œ°càz)À<:.›ô½­@žªÂ`ã?÷}}8Ð+?ÑüU›½á"?ïÿ?`h¤@¤Æ†"Ä?ûïm£Çoì?é|Ÿ5åÀ¿ïø''ì×.?ïÙ8`C·¿Üê_d"(¿ïþß~«+½?ï 'àðUNASNone?Ýâ(ç·Ð?ϸ[?r?áüëŒ$?ϸ[?r?ޗ¤2|¼?ÙìûŠ'¦?à´-æþÁ¢?ÙìûŠ'¦?Ù¥æï9-?µ4
—ÉjU?ã-}ˆcj?µ4
—ÉjU?Ò&œQ|??–ib˜"?æìÿ1×Aá?–ib˜"4FGL J1845.8-2521¿ïܲMþE/À$=:uFÔÀ9"Bþ'Q~À;Ì"ð½m@Sj¯÷)@DàÑ?º×ý­j[é?҂A©¨…@Í%îÇÉ?ô@gÌm‰?ïðcu^P¿àšdÃÎ÷¿ßn{=Ž¿â"º?+Žú¿ïšˆ!L*ü¿ï›¡æoUNASNone3FGL J1845.5-2524?•µ¥þº$A?—Eo-þ¨?ïRRÐ
.Ý?—Eo-þ©?¦làí®‡?µ j˜Hçš?î™1ÿ±%?µ j˜Hç™?§iÙ½??™`…Œ?îŽ)gâd-?™`…Ž?×Ño9|Ï?y6dˆxë?ïyAt†4?y6dˆxë4FGL J1846.0+0507?åÿ!5™Ï8@HüBÜ£À:8ÓMŽÀ<Æ
:ìe@fþ¥7§?ûIR>'5G?Ì5?ÒÓÍ?ã'-Ê=¦T@°—"ìck@`{—%  ?îž›aö¿ì´=õ.æ?Ã:öËù¾¿ÖÿÊ{
èK¿î'Ó¹PF¿âúy]¹ïzUNASNone?ڔO? w?ˑ'ÕՂ?âµ÷Ø`oÅ?ˑ'ÕՂ?âöL©ò?Õæ@à,mø?ÛôÄf¬?Õæ@à,m÷?ß×#û¨å?¸µ›?àqn+?¸µ›?áò·•Ù¼¶?» 'JHxÉ?ܐÔL†"?» 'JHxÉ4FGL J1846.9-0247c?µ 7ÿ©Öµ¿Ñ÷u¢™r'À8Ž€µÀ9þ±¨ó@ Ë´Hòb@? äçuÅ?ÊӚFgÃ^?Ú1à!é3á@LfÓs¯û@
5^†ž¿ã€¿ð©K?í§\€3—¿âp*ՖŸê¿égDýàëé¿ïþ Eð¥?ïiQ;UNASNone2FGL J1847.2-02368?Û
SÎþŽ?Úçijåeó?âyV|˜€¸?Úçijåeó?·ž¤ÌMd?Ås®¡ËêÒ?í=kfvT?Ås®¡ËêÒ?®6ŒQ¯Í?ô¼óŠ ?î—:ãÕ?ô¼óŠŸ?©•hH³? n¯,¡…©?îf©{äÏ? n¯,¡…©4FGL J1847.0-0625¿ñ""¤q¾¿ÿ-O#SÂÀ:GwÀ*ýÛÀ;Õ+y*ŽI@k÷τâþ@eXê|àü?ÏÈ÷ê‡É?àþ_o×(@¨¯bk/@Æi/œY¿ïýêªr/?ï¿©~+V¿ÏåH U5¿Û¯Cdƒ¸1¿ïiÿºùf?·Qx!$UNASNone?âÒõ"?Ì,,æÈ<?Úåæ[ÖØ?Ì,,æÈ<?êÄâ	??АÈ6?Ljï"wÛ?АÈ6?Þ}@ùœaº?ºpÈ´âo?àÁ_ƒ1Ï#?ºpÈ´âo?çícѬÝ?³´•àÒÔu?Ð%8]Ô¦E?³´•àÒÔu4FGL J1847.2-0141?ìŽÔá½ú?Ē®Bóð}À7å·lé7À9|¡|¼ê@Œè¹èC¡@ #¦Î5ƒ?Á!¯}0­G?Ö92¼î¥@}¶åû@f·Œž´a?±öí ™¿½?¦´	\u¿á ÔV.	ÿ¿é&Ébµþ¿î"]à…ç5¿ï¥íš¢®UNASNone?h…ûôã8?¦îÿRÙ|Ö?ïçzé?¦îÿRÙ|Ö?"­Çè¡>?"Qßã¶îâ?ï­Hà_é{?"Qßã¶îâ?†f ÖDàò?rÿ"d'æ??ï¦e|¦ì|?rÿ"d'æE?UŽþ‡I°?Iä˜&àЦ?ïõ8€¼|Z?Iä˜&àÐ¥4FGL J1847.2-0200c?çf¥v_W!?Z8ž'6§À8`§GØæÀ9³a°ôÿò@ †l(T@å eÑ1?Û'¾Anµ?ä'ô>UÑ@ŠÎ$»¡+@›¶‹lÛ ?í")à¤&¿ãւN8ó¿æ›»øi3¿è$nß±«ß¿êLÆ¢fFÜ¿Úöüᒁ¢UNASNone<?½¦0~·—)?Æ3a3ù¹Ã?ìK9ð)
?Æ3a3ù¹Ã?ºv²Ÿ˜Ä?Æ«h¶nËe?ì¼1)¬ç?Æ«h¶nËd?ÌýQ9©±Ë?´â|j¹?èÀ«±•"?´â|j¹? OÖTb"?˜
ᆣ&?îûš¹Ý?˜
ᆣ&4FGL J1847.7-0125?ï}¤#fϊ?ła€"¥À9PþöÅÀ:z¶ƒn@!ê
¬»à@@Ca~ ?Ï<â()?¸.žp?ïÍ4›èÿ2?û;Tiä ?¯òlÄyl(¿Ú|#¼ó'¿âð|iÝê,¿êSb}¤¿àµfÿ"s¿ß½×üÖªÇUNASNone?åäd"ÖRÑ?Ð$XYPb?Ô76ØSZ]?Ð$XYPb?äê©aγÇ?×R­ñÁ4"?Ö*­<b˜r?×R­ñÁ4"?áÂTœ,Ë?Árùôë?Ü{VǦiÇ?Árùôë?ã#\ãë?ÃÏ-¬Ùlö?Ù¹F9Øx«?ÃÏ-¬Ùlö4FGL J1847.7+3543¿èEéTÓîN@0!†¹ÃÍÀ;Ÿ¼
éÿÀ<Ͻ¥œà@!j\‹ò?ñ•:uFÔ?ÞÆÀQ>a?ì¯:€.Ž‰@P¾yLòø@Ú%ñ]É?ésÌ`@\'¿ð?í—ß…65?ïÿû˜'2¿ÞÀÝ`í²¿ïþâ~dßÔUNASNone?視›@\%?€MB©‰A?…QÙ/èöÈ?€MB©‰@?ïÜFò–s\?•'|ê}?q܆´ÆQ²?•'|ê}?ï
«'ã
¨?•KY-õ3?žJ£žK?•KY-õ3?ïo8óÜ_˜?'ºr㲟?'á"t
'?'ºr㲟4FGL J1847.7-3433?ÜyDW«OÀ,˜â~ù˜À;<Ž%ÈÀ<£yv
£W@‰nMægÓ@.Qúž—/?Ïê¯ iú?àh…à19@MZ%æC–@L¡°ƒ•?ïûñ}†=œ?ß8KgÝ_¿ÑúÍ%¸ m¿ã˜àkæ(¿ïìÇÿ]˜·¿ïÿàöO}UNASNone?çÝúäÉ¿^?ÆÃ4¾…‹?ÐD
6lF?ÆÃ4¾…‹?ӑbÇÏ ­?Ðigð'µÜ?æ7Nœ/©?Ðigð'µÜ?ٗ— 6ד?À=[
«?ã44/ä"6?À=[
«?ÑRW"
0 ?±Š»"î ?çVÔ=ùg°?±Š»"î 4FGL J1848.2-0016?ã‹IJj:¦?â™X {öÀ9@©-À:…! 8B@l¦Ð
ôà@Ó!_Ìr?ÉA¥Ãt?ÑâÊe€@XQeMa³?ñ´FÁZ}пïùÚí!+?ïðBRŠçO¿äg¿Sg†¿å`5•
Bß¿î/¢ŸÒ˜¿¿ïÿÍui8©UNASNone?º—î|–Ù?¿w¨Ây3?ì­'0m%?¿w¨Ây3?£ÊA¹8†ú?¹!#Z"ÝG?îÃ[älw?¹!#Z"ÝG?ŝ!19Å?®³ªß?꘷³¿q?®³ªß?Äk¦þ!?€ÍPÚˀn?ïˆîS¡d?€ÍPÚˀn4FGL J1848.7-6307?ìދatÀ7³c€ßÀ;Ã2ú(OªÀ<ààðp@@!›?p-d'?ýÎÇä/¿á?ÐÖ€Ú?ªó/bN?מ§Šóäi?ùÅ¡²:$?ïÿùµc#¼¿ïÿùµc#¼?ïÿN>úg¿Ôú­ÛšðÝ¿æÏW´ü¿ÚTË^b¶ÙUNASNone?ïÿȟXÖÒ>úÅèH2Ú>û°S"—IÁ>úÅèH1ú?ïópGdžº?~ŽG·"/?Yq6‹/?~ŽG·"/?ïïD2uP?eT#oüî?`»â͊°J?eT#oüá?ïŸú¬—?M@/¤äø?ˆ<TÚ H?M@/¤äø4FGL J1849.0-1826¿ìâÝKV¬åÀ-s!_ÌÀ:hÒlHþwÀ;ä"îA'›@ÇZeý
@Ïw¡øì?Ïz!™­»?ÖÔx<ҙ@@¸â4=@In+ߤ?èÃêXÎÎ?ïû³4uR'¿à¶e)O…¿è@Åø50¿ê3^1
¿¿ïÿ¶>@£UNASNone?æg¶­{?Ɛ¦ÅÒ`Ù?Ó1Û?Ɛ¦ÅÒ`Ù?íFmcý¤3?ÂQf­X—·?µÌ"àÞ_?ÂQf­X—·?ã€Oߐ­?¹2Òø‹ww?Øÿ`AÂÞ¦?¹2Òø‹ww?èó5ó_Å?± ëVwÓ?Ì3³(2€ì?± ëVwÓ4FGL J1849.4-0117?﹗Ssy°¿Â¨†z'À8T‰.‹CÀ9ž¡´N`@¿Eß]H0@'–é»ñ?ä@¯¸k?·ùf³¾3?ùg£áñø@û÷­K'F?ì"\
G`¿ážä'åp2¿è°‡A}Mß¿æ†o»y¾2¿æċë[-M¿íëÏÇSHUNASNone3FGL J1849.5-0124c?߈¿-øÝ?Ó\f¯8T?à; i÷?Ó\f¯8T?âq57qBX?ÖъºÅF?Û•'{R?ÖъºÅF?Ü@ªâw'?¹Ã¶?áßóªŽÄ7?¹Ã¶?ä!fXyDz?ÀIõ^"Ü?×½3Opœ?ÀIõ^"Ü4FGL J1849.8-0952?×¾làîK¸ÀŽÏÃøÀ:fc$'†€À;ʺà;>š@ƒ‹û¡K•@|{*BÊ?؇Ï!Éf?ï."²‡§@
†Ã%"?ùœbCÁö°?îxËrK!¿Ç<™"ü.d¿æэ'Mš¾¿ï?ërªAˆ?àc¯ga8)¿å­j0öBUNASNone?å‡ö9¦yr?Ï]²ÎY"?ÔðŒ³
?Ï]²ÎY"?âàøº"w?֐ùŠ(ԏ?Ú?Ú‹»?֐ùŠ(ԏ?Ú:sbaÜî?»zò
5?ââÆNω?»zò
6?ÏM⼁Ù?ËítËß]?è,¾ÇP߉?ËítËß]4FGL J1850.2-0201?í@à¿ã¿åg|`£®ÆÀ8ïcF÷5VÀ:#Mçê_…@ ´nÒñ	@ñhr° Å?ÆÎ8‡°ãã?‹«íë;³ñ?Ðô:$/³?þÈÍK¢Àµ?ÚºÔè$A(?ևÊ#ÐÔ¿éJÙ!ï¾ê¿éì°Ý­ð"¿ÝõÝ%O›¿áÛÇqC9;UNASNone?ÒLUÙ‡?ј¡>iá?æÙÕ@s¼?ј¡>iá?êЮ×j;?ÑAÍÓn>?ĽD¢U¿?ÑAÍÓn>?ánt­R5?Áv/*»f?Ý#¥[•Ý?Áv/*»g?ê((?æ¨e?µ03_'çŽ?Ç__e^j?µ03_'çŽ4FGL J1850.7-3126¿ØÀ©ëPç'À+@y€õ]æÀ:—žã…uöÀ<:g;x|@ùª&ڊP@ýã$ýæJ?Ò¡]•Ç?äÙ=ôWU@y…'Î?ú‹šZ‰¹R?ïêR^œ˜}¿·*1¬ËOŸ¿æˆ­'f¿çZ.I¿f³¿ïÿñ¢o+1?ê©}'QýUNASNone?ÑU<`hÔ?ÉGtGIà?çUaϷ˖?ÉGtGIà?Ð4 [Òî?Ҋ[½Wڏ?çåñïÒ‰?Ҋ[½Wڏ?Ïâ<Q÷;?±º˜J="6?è<Gpë'1?±º˜J="6?¢poÔÃâ?'¨'¼$?îØù¿sÃ?'¨'¼$4FGL J1850.8-1105¿áÜÝC'GÀ•?9ѲæÀ:yx˜˜ÚÀ<"u]@–ú©T@0#Á¦(?Ѹ:#gc<?éj܂Luú@þ"'Ùc´?üý"åø?ïüB"ßοéwKáâ8¿É*QwÁØ}¿èÑþåxÀ¿ì»4SÄ£3¿ïЋ¾dª$UNASNone?ºã0°#ª?Â÷EÐ[dÅ?죟ùéû‹?Â÷EÐ[dÅ?ÈɈ`n?ϸõ>=¡N?éͼçäy?ϸõ>=¡N?ÅÑt—˜?±š#=Š»?ꋢÿû?±š#=Š»?šˆ
Üxá?…8-)p?ï+¿'9?…8-)p4FGL J1851.0-3003?é°ׯˆÀ*BÀð¸À:ö2÷¤À<;ê'Ù²@Ú<ü@:Ü$X¤Ý?ÁY«'zC=¿°<°	š?ò1r¹[@€
Y]¿?Ð=û"ˆý¿â#¸¿ëH¶‡D¿Õ][$éÄ¿ïÿü9¡â=?ïÿì»"UNASNone?ïØÞõ¹5?"bëÜÉÎ?sö…#eO?"bëÜÉÎ?ïÈ
ÇèF?'ñäoÔé?{ùÜøš?'ñäoÔé?ï!ùö©3?' µ%3°?›ÀÁ<
ً?' µ%3¯?ïÀÿÕLBL?sHѸ'B
?€YÞٜ?sHѸ'B4FGL J1851.5+0718¿È‹(‡²Ô@
i‰¡ÑÀ9"5´í³À:ÆÃhŸý@°¯þ4ù²@ýˆ ËQ£?Àdlü'œþ?É":·¶æ@½[û©Y*?ùPx–Ó?íU]T™à¿âÄÜ=ƒN¿èº«'OP¿á`‰½®vË¿ïü¤ávR¿ïÿùµc#¼UNASNone?ÒÏ®à¤R?ËöJ1~?æð(­×?ËöJ1~?²×Öÿ^€%?½Ä€X&•©?í¥ /ü?½Ä€X&•©?×ÄÑøîþ?·$K3iA?ä—ýˆ€?·$K3iA?¬S†,Ô¤?ÆW!¹?Š?î:Ǟ-2¶?ÆW!¹?Š4FGL J1851.9-1522?퟈ˆ,À6F(}‰À:zà,À;ä€Ø´5@Vœ.t\ž@ã7!Õ<Þ?Õ\ôb=ú?íþdŸfã@7Œ†‹ŸÜ?ýkûägs,?ïï˜p"¿Ñ7è‰ø<¿èj&Ìóc¿ërH½3«¿ïÿÚÁ,/´¿ä$ð_µUNASNone?ÙÊÏln-?Îg2ö1(Œ?ã˜IÈöh?Îg2ö1(Œ?Ϲo?ҏ£³"!?è:þ?¤9?ҏ£³" ?ՅµQvH?·Äê[Ôʁ?å=}¥WDÜ?·Äê[Ôʁ?‹Šù«\.š?uV'A´4æ?ï'ÔRF?uV'A´4æ4FGL J1852.6+0203¿îʽÅ?åcl2š‡À8
 yóÀ9îäùê<I@^ô­™Ö@¬À½ÊÑ?Àâ3{ØhŒ?ÃK¤n3å@o‹XŽ6?ó,c8¯ý?ã¥üH»Zµ?Ír!²lN¿æv÷"‹Æ¿è¸€å¿ê–ß~*R¿äîDنUNASNone3FGL J1852.8+0158?¤KW%v{?À*¢-B8[?î»J¨Ÿ‰?À*¢-B8[?§öülû?¼	¦M@>H?9>`H?¼	¦M@>H?ÆØx¡*¡–?¹ËÉ(¬äU?êIá×µW›?¹ËÉ(¬äT?†¯4¸~?v,á%Ðlò?ï¥C-‰	?v,á%Ðlò4FGL J1852.6-1159¿íÇÄQæ[ÄÀ΢(´TÀ9çrüvބÀ;p££×e@h¿:­@Zñ£EêÆ?ÉSme^(ª?Åö/‡,.²?ý[ö Û­?øäC%ï}Ò?ïÜ5?ÒÓÍ¿´¨JŒk2Ô¿èûù`(´ª¿âwÆ´{G¿é¬lÚô­¼¿ïÿ¦<ådUNASNone?çø&ÞÔü?Çhk÷±Ü?ÑȲBV?Çhk÷±Ü?é£DŒ9¯/?ËË7?ÉríÏCC?ËË7?æLQÞÞªŽ?ºuk]`§G?Óg\BBªã?ºuk]`§G?Ý}	j
d?´«îÔn¤v?áA{JþzÎ?´«îÔn¤v4FGL J1853.2-0922c?íó³&ivrÀ¬¦¡¿ØÉÀ9ËÇ;"TÀ;MC0×8a@nLÂ{e&@®qÛ®ï?Ò3Ȅh¯í?Óø[{¦¿r@j ÒH7?ú¥mL¿ïÿÈ‹ñ:?ïÿY¢Ò1¿î2ái<¼¿ÁÀÒº[Ü¿éâÅA¾q¿ïüí'hr°UNASNone!?êp!ûpì*?Æv"iè?Æ?x<O\?Æv"iè?ä<2tÞ±?ÕŒœ,D?ׇ›CȞ?ÕŒœ,D?ácxþ{9?µsƱŠ?Ý9ú	Ž?µsƱŠ?Ëq8NýT4?¹G$îú?é#±ì@ªô?¹G$îú4FGL J1853.3-2447¿ÌyB'™,À&Û¦&oÖRÀ9ýìgpRÀ;µt1*Dw@ÜÓò0±@Ôa0œþ?Æ\ÜdokH?ÅҁGRÐ?ø8¸®1×@Ÿä6v?íê­ÞJ"¹?çßùÀë-¿éN¯{㦿ç–j€˜A¿ãi!—)|ѿ䍍â?UNASNone?çå-XÉ?ɶa?< ?Ñö5¥OÜo?ɶa?< ?îÙìº÷ñ?²s'h"?¢a4^`€ò?²s'h"?鈷rãK?·!2Œö÷?˙Ý"4r×?·!2Œö÷?ì•|²‡>{?£iº0?»TkÆ+?£iº04FGL J1853.6-0620¿ç Gñ¿)ÑÀ*èáÖIÀ9ÞŸ]'ùÀ;6â¿}Xñ@Ô¹¤{õÅ@ÁŒý©äj?Äá…@œ'h?Àí·(Ùº?øLZ·»+@ÿµ$¿ïþ;?ïÄÒݲù¿è‰áØT¿ß¥ý THØ¿ïýÈ[fX?ïB€®IUNASNone?îÊÓO@1B?°XŒØ‡\?£RËüëð?°XŒØ‡\?îÍ<Ø:ƒ?¹2¸$ÝÈ?£,2|WË?¹2¸$ÝÈ?餃ˆÂÔ´?·8þ?ç?ÉmñÜô­3?·8þ?ç?îBß"!?ŸëÕä[ü?«ÞR
Öýï?ŸëÕä[ü4FGL J1853.8-1107¿Ò
Z
6Ú´ÀT#;z*À:TóRr"›À;‰¼9Ҏ@méLµ:_@¼7£~ö@æ|­_I?ç!J}|­{@'«¹VÎC@%ÎÚÄU?Ñ@|g¯'?ï{ÝáÈ"¿çÛ'£²ø¿ïà.ʖ<?í®ñðs¿Þ!§ÚúâàUNASNone?í]Õ"æx?Áª+Dnôú?µÙVèÌB?Áª+Dnôú?è'>²oM?Õ6‰½µa?Ïc6BË®?Õ6‰½µa?äæa›ü?·â$×k2?Ö3=ÈÈý?·â$×k3?äd6\ç¶F?׿¬?×7"F0"t?׿¬4FGL J1854.3-3640?¶{¼ËuÀ0ZÅ;ËÀ:ÈPÓW*‰À<SAÞËÓ@$cb@.ø; ‡?Ó"ë|æ/Ÿ?ÔKÖãQª@yÀÌäJ@WIí	?Ðe0pá¬?ïîh(†¿á…ô¡'-¿Í']êâ¿îuLþ`m©¿ïüþy×ÝUNASNone?í¦"…ÎÞÅ?°ÅåÄ&8?²ËÛщ	×?°ÅåÄ&8?ê™ùƒƒ÷?ÌðRwî•Ã?Çý˜ñð#?ÌðRwî•Ã?끊çû
…?¬™;Ûý?ÁùÔ`Éê?¬™;Ûþ?çA†ªþþ?´çƒHø";?ÑÙ|òª?´çƒHø";4FGL J1854.7+0153¿ìñԜúÇ?¾·¨£L˶À7ù$(Ô4 À9ßc¨F@ÙqóbbÌ@3‹Ë{?À^®÷yɛ?Íà*w¢Ï@\E˼+•?áh­éæ@Å?æØq
"=¿ç'ö?p¿å/< B¿å»bó_¿ê†È½¯#¿ðUNASNone?Ú¿"¤¸I?ÜÒª{â÷?â 5þ­£Û?ÜÒª{â÷?‹ü…ìÔ_ê?£†ÂñÓ?ï
èL®€?£†ÂñÓ?¹ï5×òÛP?©K'Û-º(?ìÂE¤—?©K'Û-º&?8º´Wõ`?+àÅðªé?ïÿ:*]??+àÅðªé4FGL J1854.9+4054¿ÀÌ'd¸°@0Â!x÷À;>D¬Ø:¿À<jV´A»Œ@þD<ÅÙ@Ñ¢£Y?É[~€äl¿šGÚ<Õ|?ÓO*_¥,?úZu—[Ѹ?±¹YÓ[a¿î³
=Ö$d¿æ@sÝGn?Ϲ¢x`¿é\n•à¿ïÿÿ²}@UNASNone?ïÞ[7Õ1˜?i)×èD$7?pÒdg4s?i)×èD$:?ïŸEþ;Î?§¤Œ*?ˆ.€{1ƒ?§¤Œ*?ïX+˓{?‡"'&ûì?Œ)õ
!1?‡"'&ûê?ï¸èØ»ž&?s®ƒ-v"?ÅÉÑv²?s®ƒ-v"4FGL J1855.2+0756¿íQ=3A@/«NiÀ9µÕ×7‰ÚÀ:Ž~ŸBP@!ÑÞÚkq@íê‰v5ç?Æ£Þ×fXÏ¿¥Nƒ_ŠBþ?ç§Làƒbö@±ؚ‹\¿ïчF°¾y?ïÿl'ù'(¿è‰î@dô÷¿ëž¾°nÈ¿ãëæŸ‡?Ч÷à÷§UNASNone3FGL J1855.6+0753?탢`Ï?»yÎ:üÝ?³âìÿч¼?»yÎ:üÞ?î1P
.Ïß?éÎ$ª¤H?¬êÿ]?éÎ$ª¤H?è´ûêì̽?¹›Ž×Æå?Í,TLÍ?¹›Ž×Æå?ïX	ÆÞ	¸?»´QŽ²1?"þÇ$>É?»´QŽ²04FGL J1855.2+0456?ïí5ȇ?ösC>C1®À8(ܛvékÀ:ð)É'&@\àb€Ô@¦»Ò©†?¿õW°kP?ÉPx‹H@Šu¿Ÿ½ @Ê(K£—t?êœËbi¤¿Ù߀®'¿èº°ÕöA:¿ê¹ËhH¿¿í2Û>Õ}Ë¿ïÿ8$3»ïUNASNone3FGL J1855.4+0454?®'·|ˆÂ1?Á'§ÄCÛ?îԈ7sÝ?Á'§ÄCÛ?³´€Û¹—ä?Ãýÿ^Ï:7?í‰oäˆÍ?Ãýÿ^Ï:7?È!ٜˆ?°4 —[´?é÷‰˜ÿž?°4 —[´?"r©é¼õO?#<LÏ9%?ïdj°²V?#<LÏ9%4FGL J1855.3-0740?Ƅr•›ÀgϽBNÀ:$ÀwSôtÀ<…
š¶@#²…£Ã@2ƒZ'ó?Ò͖‹È¿?ﻜÞÈwÓ@5ÿñ?ü€…S'wŒ¿Ó:9LQè*¿ÂùCbÖ9¿ãle¹˜<¢¿îUĝ~U›¿ïùzu$?鉸 šê§UNASNone?Âô·Œì2?Æ]Ùu<t%?ë~'ÒÄô?Æ]Ùu<t$?Î9ö-Nj?Ò0ñ–;hö?èq'{t¬d?Ò0ñ–;hö?Á©÷WI"a?ª_F!?땂*-šç?ª_F!?Š8¼q;†?|'0âþ'?ï—;ƒ?|'0âþ'4FGL J1855.6-3603?î[kÇî	À0\'IðåÀ:ý6¤û©À<©"¾péw@ð$ÃXÚ¸@	üD~?Ò2µ^ñýß?êb–P@žӕ=ê@-}C¢—?ïÈb¥Æ!?ä̤S0ÿ|¿ØPêh¿;¿éÛÑý¹(Ö¿ïÿi'_Ž¿ïùõ÷h'UNASNone?ÄÚ½ý†«"?Âi敄j˜?êÉP€žU?Âi敄j˜?°6CDŸ.?ºq
7÷Bç?íù,W—l?ºq
7÷Bè?ÁÙÙșia?ª'ÞêH?뉉Ù¥¨?ª'ÞêH?A¼âyö½?xה&½¶?ï}òì0J?xה&½¶4FGL J1855.8+0150¿ë×EðLå¿ÁvN{c"ºÀ8¢ _ñØÀ9º`Ðû/·@ `7ûÄÜé@ܙ®'O"?Èajh©Œ¬?ÐZãü>T@phÌ›?ýq¤Ýð`¦¿å‡´Nß¿ê#| âΗ¿ÓË ¥<%¿å^ÂÞatº¿äè,ÿèX¿ðUNASNone?ÞÎP(YYQ?Ú];ÒËœ?à˜×ëÓSW?Ú];ÒËœ?¹ú«¸rµì?ÇÒíQ?ìÀªˆñ©C?ÇÒíQ?Ñç¿êûWí?µ?êõ˯{?ç 
'T	?µ?êõ˯{?²—ªì ºX?§â©2À¡?í­
¢kèµ?§â©2À¡4FGL J1856.1-1222¿íg/<‰îÀ‰"š|À9Èé<oÀ;¬‰RúxØ@nýúÂ("@ƒæœ«f?À±ÿ¦™?²Q_>e?ô'|æÛkÌ@5ՏºÉ?é2^ASÝM?ï´6Óѣ̿épÔH±¿Ó'C>™ê¿åÔcšL¿éºžÌßADUNASNone3FGL J1856.1-1217?ï»ÓÞssá?''xN–?c#–?''xN–?ïÄq œ4%? í3¢M/ï?}Ço±åíÃ? í3¢M/ï?îÓèݽb?šS~8݃?¢Î±r$)ä?šS~8݃?îAª+€v	?™˜2ÈE·°?«å]GøŸg?™˜2ÈE·¯4FGL J1856.5+1735?à˜kÎËgZ@R§¢pØ°À9¯0YddÀ;šätªÍ@žç'–òË@ù?ò^VÍ?ËéÖš9?Ïèw"KYp@Åã|;ºÁ?úqòxØÙË¿áZ΂¯rI¿æ¿‹€Ò"w¿åj¤ï81 ¿äªÅ 0!0¿ð?ïýk›Y:UNASNone?ì¦.Ôdç?¸u½Ñ?ºÏ6‰\ØË?¸u½Ñ?刋uD =?җù7œ™÷?Ôîéw¿…?җù7œ™÷?â/ÂÇÀ	?¸,ùcIï?Û¡Âzpî?¸,ùcIï?æFܶžÏ?¹ãCfÜm=?ÓrF'ÂaÝ?¹ãCfÜm=4FGL J1856.7+0125c¿ï	i‰^ßè¿à³PßìdBÀ7–|ÿ/¨À8Ö5¹ö0s@ÀÈGW@u üÏÊ?Ï(ퟀ8u?Ù&݄ªõ@MI€|'"?úCˆ¸Ë¸ü¿åە"d~?ïÈpçɨU¿Ú¬)žßԑ¿çÝÊD\P¿ïãÈ&tÞÏ?èëï<c]UNASNone4?ÂýQ¬ðí?ÓTXÍ Å?ë@«œÃÅ?ÓTXÍ Å?¤©ˆõíÌ?¸ÄɁáN?îµgp®'#?¸ÄɁáN?§fhã+?–¸e‰è0?î†ùŸIqÍ?–¸e‰è-?Z܏+Ƌ'?S²DRÀ#?ïò'¸jº?S²DRÀ#4FGL J1857.1+0056¿ï½¾¨³öD¿ë-4¶ÀñÍÀ8…äÅøÀ:c®ƒ5ª@ ±—è¥@[ àJX?ÁºuÝ&â?Úg§cܞQ@9Úak@Ò¸¯3‰Å¿ïý*,ú4?ﯴޙ}ë?¦tûTŸ"…¿ã«ón!EË¿é-¯›cž5¿ïô‡'YY8UNASNone3FGL J1857.2+0059?~«*6A8}?«ñ|›þêb?ï©«"}Ž?«ñ|›þêc?Š÷@çrJ?¡"Êkñ2?ï—Ä"üb6?¡"Êkñ2?¹ÃJ1íb?¦XÐ%—´?ìǖ¼9ÂT?¦XÐ%—´?€šíe×®?s2/Ӌi¹?tJk¨¢?s2/Ӌi¹4FGL J1857.4+0106¿ïöq+]æ¿êmjf¦'GÀ9¶)XüÀ;%ðÁž›a@ ¯®ôŸ¥@—á¸íø?Јñz+??ïÜ`w	L@h½=ã^?ó"ˆñ*Ð
?à'5Œ©Ç¿ìؑ[Ývh¿ÔbI€ýk{¿ÒtDöT0¿ì³L=pMñ¿äëIº^UNASNone?ž·þX¼Ë?¶V'p6Ù?ï
@
?Ò?¶V'p6Ù?œÝý"ÇÝ7?±ËË16ž?ïÙÁ?±ËË16ž?Çc¢ Ùq?µhTBe?ê'—ɤ?µhTBd?6qӏ"¢?+Ômñ8Àá?ïý1ÞeŽ
?+Ômñ8Àá4FGL J1857.8-3220¿ã%y™~þLÀ.¹<FØ+¦À:#õ|ï>èÀ<ëD‡Ž@Œé‡îv@†ó{??ÄoÒ Ì=Ü?Î0/ȚŽ@¢"›R×=@¥¦Z?ï'ãt®þ†¿â†?ʛD¿ãø]߯' ¿åóÂ[.пéâ6'¿ðUNASNone?å˜p›¸'D?Ç$kh
÷?ÔÏȎÛy?Ç$kh
÷?ééw!ÕM˜?ÊyˆøwD?ÈZ#xªÉ£?ÊyˆøwC?âÏطþ«?¹G¸~…?ÚxàNª?¹G¸~…?é¥ÈÇ"Ï?¦S1ù´ð¼?ˉhÜãtÅ?¦S1ù´ð¼4FGL J1858.0+0354?ë ÈxµZ`?Óу€R ·À7òŸûÆÀ9ß:Q4¥ú@*ÜGéùƒ@@öÍ0 ?º¾Ä÷@hÑ?܆—^Uö­@!
hn~bÜ@dªõ°7¿ç¿sFS¡¿¥ÁÍBC‹¿à'" ÔÇ¿ê_@z¿îJ}ғ¶¿ïðÌö%ŒUNASNone3FGL J1857.9+0355?q¯G»ãÈD?«üwìRLŠ?ïÜ¡pˆ8p?«üwìRL‹?r¿zñ?'ZjmÁt?ïځ
yûÿ?'ZjmÁt?…¬¡Užø?t€ –áíª?ï©O©z©…?t€ –áí¦?Dfn ގô?8#uàØG?ïúædwÈ\?8#uàØG4FGL J1858.0-1052?ÙD¦
WÀÙý6÷äÀ9ØB/OxäÀ;U/‰Z‡5@ý¸G"¤@dÐd1@	zg9Êüé?à7½½eQ@Y" ä¶?ôfxÚÝ1?èc]c2¿Øì#"¿ç_¿ž ß¿èÄ® 'Û_¿ê"•%–'~¿ä¤²Çë¼UNASNone?Ùýev³q<?ÑÁ©YPúà?ãMD¦Gb?ÑÁ©YPúà?áÃ|Ñ'h?ÖóÛ½y¿?ÝÒy]±1?ÖóÛ½y¿?ÔÜç
å?´	ßsx{?å'õŒzv?´	ßsx{?´Ã¸Eõ
_?Åæ¼èEG$?ígˆ÷A^´?Åæ¼èEG$4FGL J1858.3-5424¿ín\³TÑÀ6¹øã¬cÀ:*z¡†ÍåÀ<jñé¼Çœ@µ[ d¹é?ÿyfâ?¾ét£@‰?ڛaðµà!@?ŠÒVy‰@öýÝ;?z!.N¿ŸOZ±&~¿Û9NÀ­YÀ¿çㆢ›öÁ¿éA6ÌD瑿ïó³KUNASNone3FGL J1858.0-5423?Šp:Uzè?‹™̓gÚ?ï–?ª_?‹™̓gÙ?»#"¯?ýDÿ$1?ìÿ|
?ýDÿ$1?ºº"¨0?©èòyš?쨯jýü?©èòyš?DžՅ'F?ªÅî7UŸ?ꊞ¶>o?ªÅî7UŸ4FGL J1858.3-1318¿ïUw¨êÔÅÀŸU›=À:`þԆÕrÀ;÷ˆy¶¥C@Ä2¸V@ˆÏa҂ï?Îà'&ˆªß?àFƒÂ—¿¥@¯-šlþ0?ó	ú…Õ¯?ïöëN˜ˆ¿Ñ‰¦ÝNû¿äŠ&_Z¿æ,zFíû¿ïÿ®k¸µ¿¿à¿Z=¹UNASNone?Ökznj4
?Ë*0ŒJk?äÊBœ9åû?Ë*0ŒJk?ÈÕ¿r»Û?ϑ¿ºÇ/p?éʐ#Q ?ϑ¿ºÇ/p?Åøí¦Iž?±&4šJ—?êÄ–m˜~?±&4šJ—?Žv˜AEÝ?sÁK푉?ï†%Ÿ®úé?sÁK푉4FGL J1858.5-4446?ïç–ñªÀ3ì«Oœ À:vW&WƒÀ<X£Ò¿ô@²çÑ`x@ó8ÜÀ_×?Ç«µ¥é´?ÐLI'@ÃÏ,ù]O@ˆñ«©g?ïþaßîé¿àv'=\á¿âÑD£ÿ¿çg)ÚÄÝ¿ïüÍ{Hu»¿ïÿÚ@RÖgUNASNone?î˔@ž`?®f«ë˜"?£F¿ëö?®f«ë˜"?í []·ä?½Ôz£üqÞ?²ý%CÞ?½Ôz£üqÞ?èT¢xG?°ì5N©Û?Ϻ­w¶å?°ì5N©Ü?êz(¦Ï?ªB˜Ô?Æ‹]dÙ?ªB˜Ô4FGL J1858.9+3636¿à4ÃKå"@,Êl¬Ñ…À;l–+PÀ<¡gSÌ/ï@¦å‡ƒÂ@ÀµgU?Ñp˜ïO®"?äý t-Þ@?ý¾Ý ?ü>t.ûì?ìÿ¢AÞÇ¡¿ÍÛF7Fé¿áò?£%¿èñ¡Þ6¬¿ïþ' ¦Ô¿ïÿþˆ0»ŠUNASNone?Æþ<:è™L?Á¨ 1]?ê@pñEÙ­?Á¨ 1]?´O™ùÊ æ?Âé!qvë?ívÀÆ»ã?Âé!qvë?Ævg;δD?¬§_ÄhÅT?êbf1Rï?¬§_ÄhÅT?¬Vètè'$?'?±Y÷?î:'x±vÝ?'?±Y÷4FGL J1859.2-0706¿æنOÓ¸ÀÒiߗª¬À:M5fêåÀ;º©¢%YV@yc%¿,P@c8´|sï?ÓÝÂ=|¸?Ø\ø¾îì@	¦~â^.Š?ýrö6þnÛ¿ãÌÆ폻¿pjwÜÊ4±¿äÙÝ¡‰¿å•;ÁL;¿ä'̘ÊfÁ¿ïÿOÖ×èŠUNASNone?áovíZÅ?Ê0Vø»uo?Ý!%ÙJy?Ê0Vø»uo?ãr¶Ä.ø?Ӈ
p?Ù"þw¢?Ӈ
p?ݰ¬Bã'?·ÉýÐe,9?á'ž©ÞŽm?·ÉýÐe,9?ÐE§E3Z?´ßûö`û?çÝx,]fS?´ßûö`û4FGL J1859.3+0058¿ï§é_ ù.¿ôðT@Éô«À8ƒÅL¥ËÀ:7m´Zæ@ ,½¡W(@N&&v‡?Ć<¶µ^?ÈÍî_ï~Ó@•;Ãûló?ý®àË¿ïÿï~Óo©?ïÿûB«÷¿ásœ¯ÎE¿åm_[°¿ç'sýþž¿ì>†ƒ<`UNASNone3FGL J1859.6+0102?Ëfï
Pð?Ë;(Ôlø?é>fD=kÅ?Ë;(Ôlø?џ¯«¤BË?ÒÓN±Ú@?ç0(*-ޛ?ÒÓN±Ú@?ÒSèòç¯
?Àb.º:Ê?æÖ†Œ(y?Àb.º:É?ÃOn|,Ëñ?µÓÂgé9Ø?ë,$`ôÍ?µÓÂgé9Ø4FGL J1859.8+1545¿å±ŠÙ9ù@-ÙÝV‡ÌÀ:²€Þ·°ÜÀ;"''Û\@ •ù&rª@Î!¾–©$?Äk6D_«a¿´à!tK×?ó߄•%–'?ÿ«›úœê¿ï@†}ˆ?ï1KgŸV¿îû"‰µ ?¯•pkwó¿ÓûpcÀCÒ¿ÎÐE藃•UNASNone?ï_À¦?Ž´''µô^?Œ(ܖyß?Ž´''µô_?ï9@¾£KG?´ÊÖº€?˜×è+–—?´ÊÖº€?î@Œ\»A? &êÀSã?«÷:4Kî_? &êÀSâ?ï»fBƒ/T?x¨…Ó³fæ?&o_4*í?x¨…Ó³fæ4FGL J1900.4-4941?»Û 3'	À5½Å?9ѳÀ:öwZªpÀ<‰Ü°ožô@ëzPÔ@üÁr&?Ï8D,ï?×øúRAt@	ޏh"@p¾®üØ-?ïû¼¤`œù¿á§±ŸÊ¶¿ß[Á•â¿âg)¿ìêz¿ïþÕÞn_Ú¿åSu}°"îUNASNone?ïöå¸Ù?¥^Q[UÝÐ?œ¬A#HäÙ?¥^Q[UÝÐ?ëãLàêÕ#?Ç;"O¢'?ÀrÌ|T«q?Ç;"O¢'?ç'HØÃȺ?¶®-¥?ѱnNxn‰?¶®-¥?ëY­Øî ?¤<ÝU9Ó?™HœGý€?¤<ÝU9Ó4FGL J1900.4+0339?ìxï:®š¿ÕÕ° CÂMÀ8'_3l>À9í¦Ý@ø.åƘÖ@¢=ú	F?¼üÛ2k71?Õ,áàZH@IS.Ô)@TöÂ>©^?ïÿý{ÁA¿ÕbàõΤ¿ãCàµ7¿é)Ùîm¿ío¶;ÏÆ¿ïýŸÝÂUNASNone3FGL J1900.8+0337?€		'Å&?³À•pƒp™?ï¿ÛÙ¸ëe?³À•pƒp™?ˆ–qÈ?Ÿq?Öˆ2h|?8ß'?Öˆ2h|?""KÖs·w?m'Bð·?ﭲЦ1#?m'Bð·?bpËç‹	?R+ˆø–þ?ïí4=u?R+ˆø–þ4FGL J1900.7+0426?ïµ5I™¿§•TÝÊB{À7ù܄д¹À9‰W[0¨>@Û|_÷âO@tåÕ²Nœ?ÄÓ朁«?ÛpÇþ±Ì@@ õC
›Ê@"GÍÉ÷Û¿ïAhë{ä}?ï÷Œ"÷™)¿åœzŠ	ٞ¿ëj;=#¿ïÿöåv¿ïyöуóUNASNone2FGL J1901.1+0427?ÙP—8ôØ¡?ÛjÈ
:Ę?ãW´c…"¯?ÛjÈ
:Ę?…]CÞuŽ*?¢{Õ2G?慠ð†)È?¢{Õ2G?©Ø—ŽscD?œÁäÿ2Í?îbv‡ÉÍ?œÁäÿ2Í?@"L+µ±?6˜•¤ò?ïûÚìõ9Ó?6˜•¤ò4FGL J1900.9+0538?ÏeÔ3Ճ?ÞJ}ғ¶À8Kš2EÍÀ:%øÛH'@"ÞÏ®©@¤A"HG?ÈÞ½?ÚW<'W…ù@%B¯§ù@å3éf‹z?êàŒ1Ò
#¿à«µ?èM\¿è"³!*¿é"Ýr6~A¿îØú!ï"÷¿ïö[ ¸lUNASNone?€L³¤Ê‡X? ëûxtœ?ï¾Í1lÕã? ëûxtœ?Ÿ™o\'çf?²áQç«*$?ï4…èÅ?²áQç«*$?¿IÊâëÁß?¯;@Úÿña?ìÆ£¢‡Å?¯;@Úÿñ`?nÚâ‡3L?X˖0 Ì—?ïá%ñxÍ?X˖0 Ì—4FGL J1901.1+0730¿ïÂí8'¹è?ô9ÎÃG
À8Éw'ÕÀ:vnWÌp@J"á+~‰@%4åºÚ\?½ûÔ¢.=«?ÊBIP«éþ@©Ô#Ù?ø€''Þ@?ï¦~^Õ£`¿è¹Œ~($¿ãá"=‰ù>¿ä˜Õ^–¹?¿êœýýt¿ïb¾‰¬½UNASNone3FGL J1901.1+0728?Ÿ(Äâ4D?±Kñ†Z|?ï¹Øî]Ü?±Kñ†Z{?²R~R÷?éòì‹+?íµ°=<u¢?éòì‹,?Ê[hÑ»é?²\ë)¹?éi?eˑ?²\ë)¹?›üļùºþ?…›»2–|?ï Ú2(?…›»2–|4FGL J1901.2-7307?é
A´ÌÀ:"ŠT'À:Í*ô PmÀ<>é<o@FìËï?@7?Ŏ")uš¿¡¡ÛÇ*?Ü
ý¤[¢@F‹OSû*?ïù–Ys8Ý¿ë6¹ÀU›¿â¶ïö1J¿æ{þ¤Êû¿èíݾŒ˜¿ïÿ®XëTUNASNone?ïýcZI'_?7N+´I?4å-³íÍ?7N+´B?ïüçæz?ZC÷	¨ë?8ǟPÌ0?ZC÷	¨æ?ïÏØÐT?xŕ©y"@?x—ðöVb?xŕ©y">?ïîó<ÑÃ?LXN˜'ó?aÃ.ù=š?LXN˜'ä4FGL J1901.5-2208?¹Pìj¸À([åÙäÀ:ä%hoUÀ<G‰ßrï@§Z
ã@u¦uJ/?Óãĵüý?×-KþSý@Ae%?ÿôæ³]¿ï—Jy Ö?ïüŃ,oË?œ0G¤í¿åß~ØÕ¿ã®ÈáÉ¿ïÿý¡UûŠUNASNone?ïÊÄí-~7?{Up'ˆí?z‰i@äB?{Up'ˆí?îeÑúŽû'?¸Üc(.?©¢àWM?¸Üc(.?ìq†6.«t?©GiðãC?¼sÎNŠ¤g?©GiðãE?é6(²Àì?°&©+oŠ?Ë']7ôüR?°&©+o‰4FGL J1901.5-1112?Þ@î™êfÀ;õ4v)À9ÇgŽ"'¡À;g2:å¯@Á"°Soi@"Ê<ϔ'?ŎºÈ"W?¿ÇñEÒó?ö®ÀWs"\@éz"¿ïh@[9â?ï{Ø»¿åæ8¨²f¿ìB­Yiþ¡¿Õaà89'¿ïù»þHoÛUNASNone?ïô_	ô?£Ò°ß¹@,?¡tß!v?£Ò°ß¹@,?ï MVl‡º?¡pûÀ"?‡ìªdÞ?¡pûÀƒ?ë4Çچø?¯pàΓw?Ã/¸à•ä?¯pàΓw?Ž?˜Zïì¦Ð?§õæ'¾è?˜Zïì¦Ð4FGL J1901.8-0718¿èÈ\ÚLÀ}ŠÚ¹õZÀ:h'Β À<ª/@Kˆ{º
¨@$~d‰í?ËO¡¨Ü­•?ÜâÑ[|Óe@
&‹ýϤ@Áeý4ô~¿ïþ'A¶ƒµ?ïíjWŒ¯¿Ú
7`"j[¿âk8þNO¿ìÜʵ›X¿ïýÍáéOUNASNone?Ñý5_ÄT?Åaޏ:"?çqePÖ?Åaޏ:"?äÆ"ˆ=?ÒÕð>µ?Ös»îîå…?ÒÕð>µ?м0Ñ_ÃX?ºµS1SŒB?ç¡ç—PT?ºµS1SŒA?Üî±õP¸?¸Ç)—NUI?áô§W¤?¸Ç)—NUI4FGL J1902.2+0448?çv/ÄôÓп˒^;õy"À8	Î^DIÀ9¥ÙUqK@+d²Lö@ãU9î8W?ÂJüèôJÀ?Ö–ä¦è@À7OøeØ@GNs*š?ïìPU'éT¿ã†áa¯H¿âÅîAÁn¿êX/ž‹q¿í]V½{öñ¿ïÿ§µ¼UNASNone?œì8r(T?À¨~ö#Ž°?ïž<oN½?À¨~ö#Ž°?Œ=j‰¨Ã?—þB<Gh]?
UÙ]?—þB<Gh]?šô–ôB?'ÅlsŸ–
?ï/ˆ[H[~?'ÅlsŸ–?OeKîS«p?@ï`úÜà?ïø&­k?@ï`úÜß4FGL J1902.4-3417¿êÝ9#¬)FÀ0üÑc4'¿À;³*dW˜À< îؐ@¼´B½>å@elÖÂïÔ?ÐÙ¬SœŠ?ޔ¹ËhH¿@½í@?ü'Ð4`YÝ?ïÿÇ`|Aš¿Ûò¯àWîÿ¿ã³ú8?ân¿æ-ô/¿ïÿ‡4<G¯¿î^€SwvYUNASNone?îrà˜*ã?«½¿_kÁ_?¨Ñö}^Î?«½¿_kÁ_?ß»"ì9dq?ÓÁú7™œ?à"5‰ãMÈ?ÓÁú7™?âÈöwFpé?¹Ò
ŒHÉ(?Úns,?¹Ò
ŒHÉ(?Î×âQb)Ë?­]"ßBÕ|?èJk§u?­]"ßBÕ|4FGL J1902.5+0654¿ì1:ákwe?åãÆxõµ#À8ߜ‡Š£]À:q=V¢¤@þ½QYº@#Ï!?À¦cAøD?ÎBðj‹º@x¼œÓà½@-ÙçÁ¿îܼßCòÉ?îÞgߍCË¿Þns恩¹¿ãª?K¿êŒ?ÿIvÁ¿îìÎÊÔUNASNone3FGL J1902.6+0655?'"^©·uw? ›!6VnŽ?ïke
²DT? ›!6VnŽ?µ@d¯¢d?Ƌãò—[£?íWÿ"j³?Ƌãò—[£?ÀZü/ëfd?°e5¡öT
?ëé@ô&f?°e5¡öT
?Î̇'ù"?¸Ä;ýÃøš?è~LÞ6·?¸Ä;ýÃøš4FGL J1902.7-3246¿ãMžHâÙÀ0}»úëÄÀ:ÀÉÓIÀ<'oF	@dOÞ¾Š@ZR[íf ?à ð¥ïé2?Õ|8V1?øÞ<Pé'@^¬èÖC?ïü"ßphs¿ßÆí$ÒÈ¿è·ù1~'¿íÀ^à
AL¿¸¹÷2ú¿´¨¾û}å3UNASNone?ï·ÁjG?¯žÍ¶—ú?ž‰Ò½W#?¯žÍ¶—ú?ïKéÑ?±+îP1}?žւÅÞ}?±+îP1}?êi鞿ŠE?°°¾*Jœ?ÆXY…Öï?°°¾*Jœ?î[tH? ç­ Ì$'?ªO¸¾«'? ç­ Ì$'4FGL J1903.5-0825¿²—èƒ?éÀüEßÞ!‰À:½……`ýÀ;!| dŽö@µIX8¦:@/ÂÝ_Â@zU_­å?ïÿûB«÷@
?h£Wˆ}?ý[îQ"ñ¿áô€oüè¿çF©½S2,¿ã‡Í¿;Ò¿î3Ÿ¿£n…¿ï¼ú\Rn¿ïif*×DUNASNone		?é‡m&ã?Ìøȃ
§C?Éã¾Jdv?Ìøȃ
§C?æuÏډH?Ö)åÍ?ÓaÊJíq?Ö)åÍ?ހVE5?¼|®A2*U?à¿óT¿]e?¼|®A2*U?Øn
õœö?Öø6	8ì?ãÈù1"¸?Öø6	8ì4FGL J1904.0-5925¿çCf×"1äÀ8­f8C=lÀ:÷ªëÑtÒÀ<ibXº¬9@¸=Qo@ò
ú/§?Ðmn-E	?ÖüadôÌE@ð#̍ã@°StÇ'?ïû¯8gOš¿ÞEý$ÙSC¿â âiD¿éíŽ
t¿ïÿçáüú¿å¨<b5ÕUNASNone?ïkÊÀhd?–ш²Îñ?'†¼òó‹?–ш²Îñ?ë)‰J6`?È;«Þ?ÃYÚׯ&ƒ?È;«Þ?蛜|K¢?±V|3&;?͑ŽÑw‹?±V|3&<?çR8Sƒ·?°PiÉ拜?Ñ[ŽáXø?°PiÉ拜4FGL J1904.6-2713¿ï¼ä7ëÀ-tG䛬À:
Gĺ¯"À;ãW4š@×K±Ú-3@±eÆ-v[?ÅuNá|Š?¹"{?òÎ|Iýz@¨_iX^¿ÕýŽá"¿Ã¿æ<æp–¿è—Ý6§[ú¿ãÿšr¦ç¿ïY=SG¥±¿ïËBôqV"UNASNone1FGL J1904.4-2725?ïÏáLpr´?'æ®ÇíùŸ?xYÇÆ¥ó?'æ®ÇíùŸ?ïÙ¾«}ñ?"ÐFh>",?s ó*A{?"ÐFh>",?îÉo;Tt?šT´¥
Dã?£iìJ¸¾?šT´¥
Dã?¨U%æ?zyN7  ?Þ•ê¶†a?zyN7  4FGL J1904.7+0615¿å"€ènP\¿·íêÿ'ÇÃÀ8ãöíôÀ9úio/bÄ@*VgjÈK@¶ÒàD²?ӕ`˼?áDpù…@¥Y³Ð|…@º>èÉ¿ë*: bK$¿o*8sö6¿æÉäð°ä¿í­Ôï°ýc¿íÛo'C狿¿¸à[ÊÖþUNASNone
?Ÿ¡&E·/U?µ±†~F ??ïöÍÒF…?µ±†~F ??ÇQ®xøC?Ύý\,´?ê+"aùð?Ύý\,´?¼¯>\€·Á?§½ßLjôe?ìj4oé?§½ßLjôd?©R5Jƒ3'?šͅøŠè?îjÜ«WÌÎ?šͅøŠè4FGL J1904.7-0708¿ïTê"O‹À͔ÐÜüÆÀ9	wx¢À;'j¢5IŽ@)­RÞõ@3=??´ùÖ_—ý?×Òå XO¢@­H÷Q@xÀƒhTÓ?Ø÷}šµxr¿Ê!¯'Jq¾¿âHV°æ½9¿è6úh‹¿ë=¡ìNrT¿ïÿí )k3UNASNone3FGL J1904.7-0708?{4ªÀ‰6ò?{'šð¶É?ïɖª~í'?{'šð¶É?–ƒÙåß2?Ÿ¿;Ü,
Q?ïKá0×Ù?Ÿ¿;Ü,
P?ª
<Ü$àn? Ÿ¼~­-?î_\2=±ù? Ÿ¼~­-?—x$Š%–?,7Øëî?ïD?VÛ®Ó?,7Øëî4FGL J1905.2-5120?ïú™ŒRÎ|À6ï6ÍòfºÀ:E£_9MÀ;ø(/Éò'@4êv*ÿˆ@-ô!¥l6?Èg$|a$ˆ?Ìj¹ºv^@ä ¦hµ@ÿ¬ãÎF¿½¶˜>6Ö¿âL¥)ð"R¿æR¿ >yb¿æü`£®ÆR¿é›r·­¿æ£Á`]öUNASNone?ìT½èZj?¶ÙC7Ï?½Z½,¯Ø?¶ÙC7Ï?ïJ2Þ³ó?ªÎ%ðŸ«[?–¹¤<Ɂ«?ªÎ%ðŸ«[?éח†«Ç?³PsFp9?È¡¡åPãÍ?³PsFp9?í³h¹™¾?˜<ЈÔ?²dº7»2?˜<ЈÓ4FGL J1905.8+4942?¥ÖËȎpU@2'0aǛ5À:õuD× À<Àêù¾:@à¼z-Ä@»|Bp½Ø?Î\^¥§ÄÖ?é§)¥÷ß@-9–ú'è@÷bõÑ¿à±`ôâk?µ¾ñlê9¿âi`Á¶Ä¿îª5]¯Þ¿É
ý«è¿Ô®)s–БUNASNone?ì/&þ¢¢p?ÀF
~\ó?¾†È
êì…?ÀF
~\ó?îåÓä0å?¹UI$ðPé?¡¢Á¼ñ®°?¹UI$ðPé?á°Áųœ?»á¦'.J?ܞ|uî˜É?»á¦'.J?í»£O7˜?£µ([ËYá?²"å‡CE?£µ([ËYá4FGL J1906.0-1718?ïÐø'€VÀ%æFÞ	À:ÙÒÛچÊÀ<Yíð3c@
æ®bœ@#5Y~ —?Ò߂\L(?ã›bý%Z-@x~a.ï@mMÅ×U?ïŒ3Ÿ¿£o?"2ޛù' ¿¼ÄfKäZ¿äô>‹$¿ïþ
A¢a¿¿ïcoqY	UNASNone?êÂÊa­#?ÂrZtí–}?ÄôÖyKs ?ÂrZtí–}?ß_?'ÏŠ?ÓXfô]ó?àP`>˜:ø?ÓXfô]ó?á"Ñ;?½r‡¤?ÝÈüÖ]ш?½r‡¤?ÜTŽò"ˆË?·dWþ?áÕ¸†¶;œ?·dWþ4FGL J1906.1+1651?éxwh
Û@͉âlqBÀ:¦"Cƒ…À<x­"šB@ Gq=ÚÖü?þ¦öyn€ç?ÏjÜs­?ïmi?^º @\¾Fø@

 •L?ê}K…:¿î›éÕò|?åxUFƒr¿Ò&Æ0<‰¿ì³Éá`È¿ïÿÚ €UNASNone?½3†Ú߬G?Ç6~<Œ¡²?ìY$¤
w?Ç6~<Œ¡²?­f*¨è?Å/›Gjâ?î)žMUq?Å/›Gjâ?Ï¿â—Æ?ºã½ÛªL?è8PZ?ºã½ÛªL?¢.LçӁ?–©ÉÍhs?îÝ>q'É?–©ÉÍhr4FGL J1906.4-2001¿æ¬»…å6À(VÑ|^ö0À:e-Ž¯À;»üߺ[@隆~‰É@D[Ëر?×µ?¿ˆ—?ãuf´iÿx@`†R•@ðÒæl?è9€õ]县ãE;©#zY¿à†Êßâ©-¿éoÿ¢.â¿íÈ1\™¿ïà'¢ sUNASNone?֐ñßl#?˲JjŒºo?䷇Iîr?˲JjŒºo?éS ,{ì?Ë5«O$f?ʳOâS?Ë5«O$f?à0"õΈø?·tÖXx?ߟºbî?·tÖXx?ãËžÁâ?´sbh\ƒÆ?ØiÐÂ|;Í?´sbh\ƒÆ4FGL J1906.4-1757?ìïî¡¥FÀ&™
þ`ÏÀ:_¦FPFiÀ<dÍ	2¯@MÐù^$@'ùºk¡9?ÈJŸ¶i3?Ô"Ãäƾ–@†ý<× ä?ûRŠ.A²?ïôÕ?/c¿àÞ1yÏϿܗ|=¾&—¿áDêÜ0¿íÖé¡éÜ¿ïÿÞ§À£ÊUNASNone?á˓†‰IË?˲$v?ÜhØòílh?˲$v?â€vVh†?ÓøiåhÆ?ÚÿS.òâ?ÓøiåhÆ?ÞsU{^®?º%?d@?àÆrÕBP©?º%?d@?ÛYÇmT6a?´ã>"'U?âSIUäÐ?´ã>"'U4FGL J1906.9+0712¿î¼ÖëS®¿ÂöÈHٍ¥À7Ÿž;¿É¯À9Š*^x[[@ }øäWØÚ@˲5qÑÔ?µ®úS?ÉÙ×¢=×ý@A#=ó?õ· ¾œZ?í)#øÁG¿í*ÃQ#?Ùjä$'@¿ãýl§É¿êŒ<ït—'¿ì*úIݙ¤UNASNone? ¢\-œ?Á#ƒô×õ?îõÚ=/¿Ç?Á#ƒô×õ?t^@ݐ5ƒ?}'féd?ï×C~Dߖ?}'féd?¿Ÿµ"óO?­áГf]ï?ì	_{¡–?­áГf]ï?!vNj•.=?O½Ÿ¾5ý?ïþ蓇F­?O½Ÿ¾5ý4FGL J1907.0+3556¿ÝÞŠ`y@)A?À	oëÀ:؝@îÙÀ<^'ø»@Ò¨'Y.E@žº»RQ?ÐA°dmF?օ/IŒ;@$zü ¯?ÿ[Ô½0¿ïy‹Y?ïó}ü…!¿ä¶ùáØ͌¿è©H>]¿Ü2-d<?¡¿ïÿÿ" 5•UNASNone?ï1qç,Ä?Ý@	7?™ÑÃp?Ý@	6?ë€Ë$rœ?ÆÄ9"î'V?ÁüÓn5¬?ÆÄ9"î'V?꒨ö³¦µ?°Æá{'?ŵ\%1e,?°Æá{'?鱁(=u£?±ºÏ{…ò?É9û_
)w?±ºÏ{…ò4FGL J1907.7-4037?¿ÃCØ-©AÀ4.gù
wÀ:€ž<–‰DÀ<*&i U
@šã	û'@,ý>" 
?ȵ&gó¯:?ÁŽŒ	äw?ñM¿¦sœ°@¤êÕeM¿ÜÌ~VG4¿Ã¬Ö!à$˜¿èìXþÉÊ¿æ­´©^3¿ïùà#kÀ?ïªóɐØ*UNASNone?ïyÛ~Aˆ/?—M(ÁJcÈ?Ä7Îú?—M(ÁJcÉ?ï¢cqI1°?›5@{ñ;?‡g#­³"?›5@{ñ:?îQ™Sì"}?šÍ,q(ðH?ªæjÁ6È<?šÍ,q(ðG?ïo'Ò¼sý?''¡ä­
?'¨q€T?''¡ä­	4FGL J1908.7+0812¿ÊôÀÇñˆŠ¿³÷
þp]áÀ8ì8¢Þ½À:™8JÊ)@'Sæ/@'D¦">?Àé+}1Y?ÙmucÚE@VºI<‰ô?ÿP­µ"¿£Ñte6¿çUá"oA¿äÕZXTU¿êޚú—
¿ìtVÿk/¤¿ïþ=RpæUNASNone?zç!üýdd?­a‡??ïÊ1¼7?­a‡??zÙHBœ?"ŽêæN±?ïÊMoÝzÈ?"ŽêæN±?¤*tÖ¯ª°?žcK§³(a?î½X²•U?žcK§³(`?0#
8t=?"L1îÛҋ?ïýûžXñy?"L1îÛҋ4FGL J1908.8-0131¿á./èўYÀHðÄXŠÀ9,­m‹ô•À; mµ@æ@(¬ò'Ø?ÿè˜n#Ê?»KVët-?ÝÑÖÓ°@ ¸Óñ"<?ýÍBŸ¿á9|žCU¿ Î˜ÃŸ–M¿Úié=EÛ¬¿âÑeéŠs¿ï(¦G'þ¿ïþ#A"µUNASNone3FGL J1908.8-0130?YTQ,J?ZEÑ
V¹*?ïóU×iÚú?ZEÑ
V¹+?†ôÉ"3­;?"' Gs?ï¤,Ûw1K?"' Gs?†­ …Dñ©?k@½¢s½?ï¥I}êì9?k@½¢s¹?^óqä=ÁË?J¤å‹?ïð†G
á?J¤å‹4FGL J1909.2+4646¿àƒ?ínk#@0.3ðÀ;7hWØ.*À<Ö{@›å،s–@UŽäÒ?ÍÉ4¼Ë!ý?ÙT%ò{@¼éåâGˆ@?UÑ{¿Ì?	U>K¿á͊,>Ll¿Õó"\¿áæ—䍳²¿ïìRnaÝk¿ïþß06)UNASNone?èÃGô'?Á"O-Xý`?Ìòàñ/'¶?Á"O-Xý`?ãøD¹§h?Ñ;ø²m?ØvŒ±/Ê?Ñ;ø²m?ãÀsÞk‹—?ºÖL¶XH?ØC(èÒ?ºÖL¶XH?äZ昣;}?°'2w´?×J2ι‰?°'2w³4FGL J1910.1-4704¿©êß 4&À6ŠZ%"À:r·ÔCéÀ<F·`Sý®@8h§3`@J4CÔk'?Óà]7é{Y?åH-€Á±f@eöº «?öÔkçÛ¿èžç·4¿áw—±b
;¿æ¨¿aÕ2¿îì<fd¿ð?ðUNASNone?ïÛ¬c,VÔ?‰YÄ5µèˆ?r)ÎiԖF?‰YÄ5µèˆ?땦p"?Î&GÆ}9?É«f=µ?Î&GÆ}9?èñ°üä?®r^‹Œ?Ì9?"¤m?®r^‹?ãšrð_®·?Á̅'­^¥?ØË@¢'?Á̅'­^¥4FGL J1910.2+0904c?åQ
ìΎ_?5ïò<4üÀ8Dß-!¡À9òŽù,§(@!;êH³£@PwDŽ¥?ÀZyɹå?£¯a#}Õæ?ô0ÓÊ?ú$ÉâοïšG©â¼ù?ïÿd™ÝŒ8¿åµ)ã(Xå¿Ø•ýB`wº¿ëH¸ ÅÝſаh¾‡úUNASNone$?ÌBèÙ"Í?ÍÇ{VM?èïEɸ·M?ÍÇ{VM?Í\擡LÇ?Ô6@º'Â?è¨Æ[¬Ï?Ô6@º'Â?ß!jr ß?»¥"
q=¾?ào}JƯ?»¥"
q=¾?Í(v
ó×?Á3׉ž?è¾uâ}C
?Á3׉ž4FGL J1910.7-5320¿Õwoå¦öAÀ8>A_EàµÀ:~ùc<À<b
@@M…XÄè'@$$D'æÐ?Å6w
x~í?ُã¢Ò'€@•›Þwì?øöûú·Á£¿è›n»Ÿ}ß¿Å£œQÚ¾¿ä6žÂÎFJ¿çGú D®†¿îÒWPHí°?Ҕ«]¼HÆUNASNone3FGL J1911.1-5318?¥¼tØnPÊ?¥z_þñë?î¤8²yô?¥z_þñë?×ã¶.žÊ?ԃ'Õ^Ëp?ä$èþ°›?ԃ'Õ^Ëp?¿Hs+3È?¬žìí3Ë?ìñšœY‡?¬žìí3Ë?¹$ñmç©?¡Vô"¿
Â?ìÛaÒC
ß?¡Vô"¿
Â4FGL J1910.8+6300?ì^œs4@5Ø6¸ù±1À;eszK¹À<åyéÐé'@ .e2§?ÿ`UÆ2o?ÌC">™BÝ?ö©à8º\?ôˆ²ÁˆÌ@{2ü+µ?í‰?MóÔ¿ï韛†&?ïÄ÷u³¿åÎéõÒ¿ÖÍY$3ü¿ïÿÕ7ÕYcUNASNone?ïõ10"#? -ã:¸BZ?U՝Ÿ»»9? -ã:¸BZ?ïüúfT›?TJŠû.ò?8,Í['EO?TJŠû.ò?ï֝ÔÛ½q?v…±Dv?t±'!G"?v…±Dv?ïîà€8‰<?V…؍ÔR?aÇvÃN?V…؍ÔR4FGL J1911.1-3221?ÛS΃"wãÀ1ùÊâ°À:À1"öÂjÀ<BWڎV@í§¸Á'@Ñ>Eþ?ÑZ¨VÌ?Ԁo|Ä>@H÷}z"@ÙÙ7"@ê?é÷•ÞN)"?ãâ`b@fø¿àî`/뀿áñĞ*"¿îŸg~¿M³¿ïý"€U$öUNASNone?í\õGß`+?±ƒ	_`0?µUÁþ°?±ƒ	_`0?îÕÖk0º¯?´J{ÆԆ?¢¢™LôU?´J{ÆԆ?ë]ý­®m?©
ZZ©ñ?ˆ	IFK¤?©
ZZ©ñ?줝°Õ
d?¡mÛäÇ?ºÛyW¬Ý?¡mÛäÇ4FGL J1911.3+1055?ã#P°ÊËÀ?ãgpQ¡³À99ˆ{¯¤À:•¦†è½@¡'Œ_t@íŒ_õ3?ÚBj?ÒËÊCZ°@r=äg?ú=k€3í¿ïõ¥¾Àðv?ïÿŽñ ¿çHÌAâx†¿çË,^WÏ¿í8="ßEu¿ïüÙçUNASNone?Èp'¯˜?ÆM†Îfj?éãÛTܼ?ÆM†Îfj?¥T"Èìÿ?µü6å¯?³q0?µü6å¯?Ì4V–À›Ù?³6nˆŠ?èòêZOÙ
?³6nˆ‰?Ÿ1/?זñ?"Ÿ¬òŸ¨?ïv†CJ?"Ÿ¬òŸ¨4FGL J1911.4-4856¿íÄ\¯lGÀ7B«%(®À;5Ÿ>HÀÀ<óK¯Ri@vǕ«Mv?ÿ-gwžZ?Ðþ!ÃõÝ?èIè^9q@àýÜ9Q@ÊÇU> Ð?™cÿÙ¿y}? N>§?ÄHôe˜
M¿åÂ2᱿ïÿ;2G?߉ˆ>þB'UNASNone?È^eŠÑ?ÆÐh3®¯Ý?éèx~æL?ÆÐh3®¯Ý?×î'a¹™n?ÔEñxµñË?ä¶Ï#3J?ÔEñxµñË?Ãoj_yô?±ø‡iá¯?ë$%xh!ƒ?±ø‡iá¯?Ò¾÷&§ƒ?µ˜"jà?£?栄l¬>??µ˜"jà?£4FGL J1911.8+1447¿Ò[ôÀ¤ž,@?ºÆà$À:-±4ÀÑíÀ;{miç@!A×0}÷'@˜¤§Ö?Âå9?¼®r¿—}4E?ÔïäÿÉy[@æÊ6Åcø?äE~Åý0¿á®å%‰&…¿çÅàŸgŽÚ¿è–•Ù¹¿¥¢¿76¿â›`^©UNASNone?ï yƒI3j?ƒŒŒ€Ò?‡áŸ-³%G?ƒŒŒ€Ñ?ïßÊç$ì?"üþMARÒ?pŒríŠÊ?"üþMARÓ?î…v=©?šdÕ¹Ü?§®øœ/õb?šdÕ¹Ü?ï°Íé†pš?xCè±?ƒÌ…žcÙÅ?xCè±4FGL J1912.0+0927?î°7Ò¡¶ä¿Ìæ'Ú]"À8ÓbÀ:ÉîËû@Ÿ¼wjÏ@£ß¾AÏ?Ëṳ́ÞÇ ?Ô~ÊuÚw°@DG!ý€Ê?õiҩۆ#?ÑώH,¿|¿æ…¦2.Pu¿â¿-§Ù¿æÛWãä¿ïi§Šóä¿éb`¢­ŸUNASNone?œI‡;Ez?¬¯2Â?ï³Æ%Ô/?¬¯2Â?·$!%85?ÅÈG¤ªfš?í{Û\øú?ÅÈG¤ªfš?±¢»ÍyH?¢—'Lš›z?í˨œfP×?¢—'Lš›{?omK¨)ûT?_qO)Èù?ïà'´WÖ?_qO)Èù4FGL J1912.2-3636?àƒƒæPDÀ3­Hˆ/À9û‰ø;æ`À;n'å".(@t9)ÂF6@§%?Tª?Ð^?ÜV?ϑ+6¯Æ@ëÅÃď@þü—À¦y?îÚ)'z¿ÕLÉè=ì¿éô§<‹Â¿éœhKBôq¿ëò`°
¿ÑŒ'Á)iUNASNone?å§;¤á?É¡ÙæPÊE?Ô±ˆ¶=ùô?É¡ÙæPÊE?马	_?Ïõ½èŠü?ËåYO«Úƒ?Ïõ½èŠû?ákÍ.,?·áÿÈxÙå?Ý)Äe£§×?·áÿÈxÙç?â'`èo ?µùD
öÖ?Úû>/ó Á?µùD
öÖ4FGL J1912.2+3621?Ö%Ç| XÒ@'¬ì O*àÀ;˜Ø?ǖ,À<Ôe›eK´@(p¬@» ÒÞ_?Ü!3 ¾¼i?îbÑ¡GãÄ@
qU'Ù‹ø?þ:ñbÙ>?îAŸÝ€y¿ÓáP|ð§¿ÌËD˜¿ì·c^t)ž¿ïÿÞý¦ßR¿ï÷@s–VUNASNone?߅Bþälé?ÍÈ›aL?à=^€É‹?ÍÈ›aL?Ók6|DÞM?Ó±"Ú	³?æJdÁݐÚ?Ó±"Ú	³?âºsÞ±Íß?·\"¾Ö?ڋBœdB?·\"¾Ö?®Škð$ô?–{ó½VÆ?îY@ý¶!?–{ó½VÆ4FGL J1912.5+1320¿ïì²%@3è?÷*ՖŸêÀ90‹µ«HÀ:ºðY|s@Ý$zØç@
¸·a+?ÇÅÿ©?ÔæÈ •¡½@àÆÜÈÃS?ýݹ\~0?é"Ë ¥<¿âõ:ªù›¿ç)ë‹Ô´ù¿ê^æ?d™Þ¿ïø~eET¿ïзþ^•7UNASNone?½'(7øœ?»â°é 9?ìMºùÀí?»â°é 8?ÁíÙúíMß?̗›`ÞÓa?넉D¬‡?̗›`ÞÓa?Êײ>»<?±´£/Á>ž?éJpzQ1?±´£/Á>ž?£ò"3ܤ?ŠÌ/¯?îÀÖΜÂ5?ŠÌ/¯4FGL J1912.7+4610¿Éë1¶·Çå@/rÿÑÜ×À:Ï7Žâ†rÀ<¤¦Æ¨Æ]@W˜·Š @¬À½ÊÑ?Ŭï¢9Ñ2?×
;|Øæ@®0‡‡H^@0X,¼Ìz¿ÑŒž
²?ïcìÊì"¿á­˜‰Ï!;¿à—Lg"t¿ë!á1ßÈ¿ïÿý¡UûŠUNASNone3FGL J1912.7+4610?ÍóLSN'`?焎ñ°²?èƒ,ë,[h?焎ñ°²?Þ¶ŸEã?Ôð#hÎÎV?र}{Ý?Ôð#hÎÎV?ÉYÃç?‰?²Ý·0Ӕ?驏0>Þ?²Ý·0ӕ?à'<½¡í?´t)©íì~?Þۆ…Ú¼'?´t)©íì~4FGL J1912.7+0957?ï1Ð4Ã¿Â¡«`ìSüÀ8™‰!|QŠÀ9ÿ¦sœ¯Ï@>Ž2Þ#·@æÕw–?É;΢ºÕ~?×B-'ð
@~Ò`Š"S@Œ1>fm¿îô‡%ùŽÍ?ïÐý¤-¿åȪ(]\¿çò—a°õ¿ïrÂ)ۛ?±	5ô–UNASNone?¢mIj?Àr.½û™@?îÙ/ûi^?Àr.½û™@? LÙ øâ?µá‡~ÑQ©?îÿ;2eðr?µá‡~ÑQ©?§aóˑB?˜µæe¸à¼?î‰îÀÃFì?˜µæe¸à»?~&³ÂBRÛ?tk>ôåÐ?ïò˜{{Z?tk>ôåÐ4FGL J1913.4-1526¿ëL"ÝF À'}ÚH¶R7À:¤$'–GÖÀ<ƒ¶85Ñs@¤¬é¶¹?ý+oðS?Ïd'œÒK?æðbžZÉz@‹&|k‹i@)WÅ8Ù»?ïéϘY(?ÒÝ¢] w¿»4J	Žt"¿àçÏAǺ¿ïùŒž^z_¿îTœÚ–¹ëUNASNone?¶¶[€º6>?µÌšøBÏG?í)4è¹8?µÌšøBÏG?¦0úUŠ*?¯A P³?îœðZ§]`?¯A P³?µ;Éfb‰:?¢I…ƒ¾÷$?íX†Ó3®Ù?¢I…ƒ¾÷#?¬›@k+^?"¼©|% ?î6KùNmJ?"¼©|% 4FGL J1913.4-2652¿Ô7½l£/(À0c÷œ"/¥À:ºØ´5&À<cAfҜð@ž«¼±Ì–@œ':×lc?ÖiÀãàd¯?ïГ*êU@؍]b²?öô¾
'*:?ïîj}L¿Ö´¯àÄ¿ê†Jg,_¿ïõþ~pH¿èup¾®ý¿ï‰:;e0ÜUNASNone?ì'ÿ'r ÷?òâÏeÙ?¾ÀìjøJ?òâÏeÙ?ÑÑ<Ÿú?ÓÎzÙNcÌ?çaôv°?ÓÎzÙNcÌ?àb£í1œ?¸å©'Ÿ?ß:¸%˜Ê?¸å©'Ÿ?ˆXﳘÕ?€Vίѩ¡?A3¡?€Vίѩ¡4FGL J1913.5-0923¿Ò÷tùÀ"FQ	¿À:?þ@_ŠÀ;œò™åï´@OcJµ†@fnŽ›9?Æù¬¿;>Å?¡ç®ƒMî?Û⍩K@ϒ¾^¿Ð¸W_bf'¿æ ñ—‡q¿ìðŽ]{[@¿ÛÓ&Á½¥¿ë[Ë}lg\¿£f_Î@UNASNone?ï'Ýxrw?a²ßù"?‹H¡üãb(?a²ßù"?ï÷ÃT
?oð
fíKþ?QÐyWËä¸?oð
fíL?î8â€J~Ù? NYÂ*(?¬q×ûXs? NYÂ*(?ïá­Öìš?\ôòòNü?nÿR)ef?\ôòòNö4FGL J1914.6-1157?î.ÀK†²ÅÀ%È%žÀ:Ë©·À;'gÞ5ªÝ@¼3ù¬©Â@ðRãÒ¢Ð?Ì)³ʅu?Öﺢþ)@Oá|‡:?ÿՐx2Áž?ï±åàïïg¿æYôhI¿â­[þX‹¿ëA«"ªO¿ð?ïû÷"IôUNASNone?é›[$¸'¥?ÇÓ!@ûî?ɒ"mao?ÇÓ!@ûï?ÞÓ(ÏÈî?Õ}j($ëõ?à–k˜u›‰?Õ}j($ëõ?Ød0ºuz¼?¸õ)›´_Ý?ãÍç¢ÅB¢?¸õ)›´_Ý?ÚI"ÂÓ`B?À4™½ÜÛ§?âÛ=ž–Oà?À4™½ÜÛ§4FGL J1914.7+1012c?èÕ×zmNþ¿Ý3qÜç!7À8ÎFèòAÀ:6Ô­kÞu@OîýNIå@•ÁF†Í?ˬâa3¡˜?Ð+ØËސD@	]5<ø®Ó?â8èDU"$¿æ»/€÷e?ïõ8áÈÝT¿èÛª¶!¿æš¶š[`y¿æÄI,«¿ï—ªÝŽ¼UNASNone8?Ö§=Øah?ÖÏ'ÛBG?ä¬aÏKú?ÖÏ'ÛBG?±zô½/;?ï?Þ Q?íСhZ?ï?Þ Q?ÏbÄ?Ÿ)©?´Wô²?è'Nð5–?´Wô²?fŽ	ζµ?[þšÝƒ‹?ïéqö<qJ?[þšÝƒ‹4FGL J1916.8-3025?ÔÝa2› À2k‡	VÁÀ9ÀUWJi±À<2š†ÿ@ך¤["{?ü¡m¾I|K?¼((¾DÁ?Ñ|vžÏ@pÛjË?ùt(ì]`ٿ䇱°¿ã­¥àNß·¿Êf€Ä`˜¿Ü;Bö…¿êþþ"ZGõ¿æã"GþqUNASNone3FGL J1917.1-3024?°á'íÔ?®qª¿c™?íãÎ_†?®qª¿c˜?ºD*x8<:?Å2ø½£äy?ì·z°øøy?Å2ø½£äy?¼Ø'Â¢?¨OõÔs?ìd﮾l?¨OõÔt?Ç!-6"Ã?¬?·d³•?ê7´²_·P?¬?·d³•4FGL J1917.6+2609¿ëBΈÈÜ@BèbTˆîÀ:\p\‰mÒÀ;ű܆~4@šš"P1F@§Jº8u'?ÅmbÁ_?œš±,ç?ÊL齞\?ñ'ç[ne¹?ïþ.H‰Ý¿æ»áWžL‡¿ëÄþÍ%¿èÄ$½Nªˆ¿ÒZaueݪ¿Û3Üȃ<UNASNone?ïÆÜí]4ç?ˆXΚÂ?|'‰QeŒ?ˆXΚÂ?íÙ¥xÄÕ?ÁÜ*lß?±7jÔ9ÙX?ÁÜ*lß?íî¼®«U­? A\?n¤J?°ŠŠ¥R˜? A\?n¤J?î&]œœ?ž,ŠÏÅî'?­ž&6öN?ž,ŠÏÅî'4FGL J1917.6-3204?îY}ÔRÑtÀ3*0"ÝzšÀ:CbzH›zÀ<*.y@-·qEèm@v"aKts?ÈS7_'·¨?о‰]aZ
@X/ž‹q?ý²-V?ï¹#!ÃM¿å]ñLÞÕä¿Þæg}'§ã¿çh¼LLí¿ê–`ÿõE¿ïÿ™s,ÛUNASNone?ém.
å"å?×Èåûä`?ÊKGÔiìm?×Èåûä_?êÅòÝ1{g?ɖÍ5NX>?Äè4‹:^?ɖÍ5NX>?åGߍb?¶7ndqö?Õÿp@äý<?¶7ndqö?å6D̟Ûo?²êûþû?ՓvfÀI!?²êûþû4FGL J1918.6-7813c¿ÛÆ7ÈcôDÀ;æ·ª%ÙÀ:yl2š‡À<$aX"@ѧ*{ԍ@±ƒÞFqÔ?Ó@¼Þ˜&R?׈^2æ1?ûßFfìž#@Œ G2Ä?ï¾
'*:¿ÓíIå&_æ¿é´â_ܪ¿îú´|lb?з,<f¿ï¥c¯˜	UNASNone3FGL J1925.8-7826$?ïvYŠµr
?›hÜuÐ?'4ΩQ¾Q?›hÜuÐ?ïî"f—È°?™ÖäÊîŠ?a{™h7OŠ?™ÖäÊîŠ?è}ÙpΆ?µcŠîè¦ã?Κ<Åçº?µcŠîè¦ã?ïºrewº?yDIxˆ?cf¢Á?yDIx‹4FGL J1919.4+1313¿çd¡w"T¿µàK¯«ÕÀ8YÂÅ+À9úád3†?@ïf£M!œ@w$ÄÛfÄ?Èڌ(õe?ÞUœŸ]}ß@žK¢•Áž?ÿQünûá7?ïï>ÜÇ?® ÃDõ1¿è'âôV¿íœáL¶'ø¿ïÿ¥!b%d?ïøDRëUNASNone?ès—ٙg?ÔSñÿÑÇR?Î1£ ™šc?ÔSñÿÑÇR?¯äqzÈ?͖4¡Ú–À?ëTã¡Mø?͖4¡Ú–Á?Ôinž{'?µ¿Ýf'°]?åËH°Â>Á?µ¿Ýf'°\?qȄÜ*R?eØœ.ï?ïÜnöGñ¬?eØœ.î4FGL J1920.0-2622?åç}®À1"ÙºÀ:MV¿)vÀ<V'Tà@.ô®¾@I}<kÁ?Ç׫£Ì?Ò¡ä@Ü¿@
ª"Àā@4æv"1?ð?Ð'UØy©¿ãŽO¹{·¿åÀÌäIÁ¿ìˆ[NoÑ¿Ñ&w ÈÍUNASNone?Öhn$þ=?Ê+¦Çä?äËÈí€áw?Ê+¦Çä?à¾ÊÙ¼é?Ñ©Ø잰¯?ނjL†ü-?Ñ©Ø잰¯?Ö¥|kzä}?¹NP
™z?ä­AÊBÂ?¹NP
™z?àπöxêÍ?³S\&vŠb?Þ`þ*f?³S\&vŠb4FGL J1920.7+1334¿×qAIïþI¿È‰S¦EN"À9Êc&3À;vރ®uÊ@/ Ô ~%@Á›@bƟ?×ÓDç:·?ï•ÆÁ#@9Ë@D†r'&?ì®rn²e¿îZièÑæ?ÀË(²Ñ¤¿ê€ïHø—V¿ï÷Ú,0às¿ïÿüÉï£UNASNone?ÁžšøÚ-Ä?Ũe-|O?ë˜YAÉtŽ?Ũe-|O?Â@9Ö<¸e?ÍñÞªE?ëoñŠpÑæ?ÍñÞªD?Ñ,Ï­!Wp?³TRXxJ?çi˜)oTH?³TRXxJ?'ôìÂ/…#?ƒ"|ößÞÁ?ïpX™îƒ×?ƒ"|ößÞÁ4FGL J1922.4+1453c?ê¹æòä'?­ºãôº/À8ɼHKÀ:%ç}R@ó¨9Dš9@©K£l3?ÐTa¡Z®!?ÚAœ¬s'@‰¤Òh@
‰ºr¿íxÚÂXՄ¿™¼S`'Õ;¿çJè3FS¿êÙ๨¿îª,ŽÔD¿ðUNASNone8?Öak]öÇ?Ûíaíøŏ?äÏ|JQ?Ûíaíøŏ?­÷Cx¯¢7?À"‰…Ð?î ‹ÈuÝ?À"‰…Ð?¼«ïš‹(X?§åË?ìj'®šö?§åË?–?ˆ\râ9?‡}%Åتí?ïN½hï?‡}%Åتí4FGL J1922.5-5233?é"'.°ÀÀ9͋¤
âÀ:w¢'^<À<tñ´âg@ ÖQ…Ú@M œÃ?Ç6E¡ÊÀƒ?Ñ2%acr@@™'6@3{ùö{?îú÷íâÇ
¿Ê$ï"¸Ó¿áæüŽ[wö¿éC>n$Ì¿ét(%¸÷-¿ïý–-ÔN¡UNASNone?îx®N?§DUv4ƒ?¨~E~k)?§DUv4ƒ?ïÓØÂä܇?‰çc÷ûl?vž'¼<?‰çc÷ûm?ë$M<
?©Ï/Qó?ÃnËëÕ?©Ï/Qó?î–}óucC?%<óÉD?¦˜ È©ËÍ?%<óÉD4FGL J1922.7+1428c?ãYx!$™¿ÊGBIP«êÀ89Ý3L]§À9†2Áô+¶@¥¿Ü#å@U>Lò?Ê&n©«àn?ÙÂÓº&×Û@ý8bGõ?ûvýz#Ý?ëˏJ‹>¿æ2Ï˄Î0¿â•ýÍö˜x¿éjª}ík©¿ïÿRáNd?ïÆ+B£éUNASNone4?ßÿšRÐES?ÛkõÌ3›?à2֗ÝW?ÛkõÌ3›?¿ˆ†ºuÕ?ÊÃÈ"`ï?ìîO(±F?ÊÃÈ"`ï?®üt½
ÊÕ?¢sžýæ?î8´/#R?¢sžýæ?f‡"]hâ?_Á'þ–?ïéxk¢—p?_Á'þ–4FGL J1924.3+1601c?éºÐÞ}¬?ÉÎ81ʨÀ9uk¼ç|À:UùÖñý@ºE?Ð$›@8圧k?Ñ*YÛ=¨Ø?È.1× ì@IÄo0:?úٔ¾¾l7¿ÒñõNÌ?ï½Ë½ƒ-ǿ燊£\'¿é´ãÅ˜¿ãg†àzª¿ðUNASNone8?ÕÈjåþ%?Ѳj˔Æ?åÊú
î?Ѳj˔Æ?¦6Ԃ" ?²Á¾ÿ%×n?·ÝÖ?²Á¾ÿ%×n?Ó8ø;>?¸ï#rÞ"?æcùž#â`?¸ï#rÞ!?³ñÚPnx/?©M™lV$˜?íÄµò0ú?©M™lV$˜4FGL J1924.3+1628?àIP!_ëø?Úb<5:tÀ:k÷ÉЙ
À;'§WÈ=ò@#¾%7Çíj?ö·zU0³ý?Ñ£_ Ïmç?Æõa€ùd°?ì5J¿ì¿†?øߣ¡…KY?æt$'/¾¿ìW<'<ZÏ¿ßhŠãžJƒ¿âkÂ[YÂê¿Ù驼ÒXÓ?ȳùAI÷UNASNone?ﶧ"¼±þ?""ý9ó'?'VÐӀ?""ý9ó'?í¿‹¡]-?Æ׫	l?²K¢õ"?Æ׫	l?í#kg f?¥Èæ÷—	¦?·¦ä¤ÂüÑ?¥Èæ÷—	¦?í‹û™K‰?«+¸hÃAì?³ #7£¹?«+¸hÃAí4FGL J1924.8-1035¿Ûÿ$.|éÀ(V>ò"{À9۰݂ývÀ;éü7ôc@™ÊM²o@Мe%õ?¯fõØ^Ñ?Þ{üOÇ>@>+ —ºœ@áù&Çêæ?ïé‹$£M¿ÓgÃþÇñœ¿Ý@`") ¿ß
)N­âý¿î'x_7H¿ïþ!†ù"UNASNone3FGL J1924.8-1034?lM'[¦³î?jHî5¨DÀ?ïã²Ø¤YL?jHî5¨DÀ?'Ü2ßn¤?–ZÂ&m?ïiîi‹?–ZÂ&m?'^.sh]?†B˜ˆÆ,?ïm$d¼?†B˜ˆÆ/?Œ"WxÛLB?sÙùqÏÀ?¢'Ï?sÙùqÏÀ4FGL J1925.3+1522c?&m§=¿Ô"j…¯×ÊÀ8ۚ<VÈdÀ:@æp–@òµxrW‹@´ØŸhæs?Èñ7¥³®C?Ösâû¸G°@‹7T*?ÿ'Ú7Äg?ԊÿbvAÑ¿æË ýP£¿å·cyL8¿èàyAàJ-¿ð?ðUNASNone8?Ó®ëÖq??Ñcñy¼ë§?æ(ŠôG`?Ñcñy¼ë§?Ñö¦¡á ?ԊïT ‹?笯?q?ԊïT ‹?Äll™Ø…?°MÑ·¨{™?êääىøß?°MÑ·¨{™? 1ͧnF?"®ÿ98?îüî³%‰?"®ÿ984FGL J1925.4+1616?áò¶'êGv?µä³HlUiÀ8+YhQ"2À:1°Ÿoœp@ @Ÿµ½f¨@ÈÌW\h?¶DË+­?¹=§UnòQ@Ž­…èÝ?ý´ý2p?®?ÅdÞ{öÆp?ïÊSá(¤d¿äV5@Ԇ€¿çÖÔÃ;S"¿å;$,/3¿à+Žž¾Ç{UNASNone?ÄSîV–U*?Ë(úYqÏ×?êëjZj¶?Ë(úYqÏ×?•›Áa¯%²?£eàíù2C?ïS!ôò†Ó?£eàíù2C?ÎEÒv\"å?ƟÄÈNJW?èn‹bh÷G?ƟÄÈNJW?°yæuÐ`?¥'LzN~¯?íðÃ1]…ô?¥'LzN~¯4FGL J1926.4+1602?ä;ENœ•¿Ïþ^Õ£`À8)çZÍÀ:*{¥t@^ŽÄÔ[@úv¾£>^?Âiž1Žm?Æ¥˜*ƒ·/@
‹}ý[àÑ?üÙ,|4ÙÑ?ïhD¢qYŠ¿áhÈv%÷¿åeŸ—	œ¿æñÑiÀ¿èEþFÂ\1¿àúsÅÊzUNASNone1FGL J1926.1+1601c?¤°Ò#þ?«Ë{&ïxš?î´òÝÆ ?«Ë{&ïxš?ÂVi1Î'?ɽ<úÈ^?ëje³Œzœ?ɽ<úÈ^?ÊÏåÂ®?¹ÍVÕNÓ?éL?†œT?¹ÍVÕNÓ?¦€á¬BBÉ?"š:wÏê¦?î—ñå;ÛÔ?"š:wÏê¦4FGL J1927.4+0253¿×'¶Š"cÀ·tî¿eÜÀ:nš»É.À;îjCk@5w>Cˆ@GEÙþäw?Ñk€'Í?å{h÷:^¡@tu½ò>v@~?NI¿Ù|½ÀÀO¿Ö†/¤³S)¿â2•"´¿ë u¡æv¿ïÿ{Ûèt?ïú!Dô&UNASNone?֍<Àôy;?ËôJëßs=?ä¹aŸ…Ãb?ËôJëßs=?åäRƒ¼æÈ?Òj#B^?Ô7Zø†2s?Òj#B^?ÐUÍù»?¼»I¡Þw?çÕ"w¸?¼»I¡Þw?æD麈+®?ºaÿ!á1ñ?Óv,Šï¨¤?ºaÿ!á1ñ4FGL J1929.0+1729¿è«=Ž\Æ%¿¶Ÿ_´ÆqÀ8<ó˜:õÀ::&¨á5:@Tó®N@ ,Æ1¨?ººdë<#?ÕPâC5à@ôH!ˆ@+sxó†Ë?ï'ÞŸ]'ù¿Ö«³¢"NÚ¿ä¶b'$-¿è†"Ú8+¿îDl@šúÿïÎ$ É8ÄUNASNone?k)܄gÑá?oQ§³O?ïäÖ#{˜-?oQ§³O?'±°,g¦?X8žÐcá?ïÀڜŸ§1?X8žÐcá?£Òx<*Ã?ž ñ7­ðä?îÏ2Ø|=T?ž ñ7­ðã?Wmè".{?HHs+Ñô?ïôIt‹îè?HHs+Ñõ4FGL J1931.0+1754c¿ïàõé%™Z¿Ó†oE],VÀ92ð¤BjÀ:‡4éد@ê''¸@_Ëâ˜@(öÎþÖ4?ÒÎBXõ»@
…凮¶@öˆþð?ïë@öjU?âA¦=—¿çuݜþ¨è¿çdœ,ý¿êϯj¼6}¿ïý "DsUNASNone8?Ó	Q°^R¨?ÒRß
ÐXE?æ{W'ÐÖ¬?ÒRß
ÐXE?ɒòXa¢ø?Ҙ¬ ¯F?é›Ciç—B?Ҙ¬ ¯F?Ñ{î÷€N'?µ–7hÈ­?çB"?ض?µ–7hÈ­?ÁߛŸ‰>¦?ǏÝžÄ-?눰V?ǏÝžÄ-4FGL J1931.1+1656¿ã1 °©˜û¿éew•ÜvÀ8k§AøÈÔÀ:£ùnì@é'"§ŸÂ@蓂(cÌ?¸3žèãÙ¯?Øf¨@%‰ý@7Ý÷vÅ?ùõzÞm‰?ïÕM9Æö¿ÝËØü0Á¿ã£˜ ö/G¿é ÝDU¿ío³íöz¿ïàåõ"UNASNone3FGL J1931.1+1659?a%[²Þ?ÖíüKþ?ïîÚ¤M!=?ÖíüKþ?~Nè¿?•*<(	é?ïÃc÷Ðü/?•*<(	ç?&ë¤ñî?…ʘ£&ñ?ï¾È¢Øq?…ʘ£&ñ?&Ù¼\¸éº?, Rb¦Ð?ïþ'd:4q?, Rb¦Ð4FGL J1933.4-2711?ì€å¿ÏíyÀ4§ã\[J©À:]«p_À<€»|Bq@k"§ïó˜@)ô?Ø]$?ÈÍfOÀ1´?ͪxúgº¤@à±5—''?øÓÁñQ'm?ïøU¦P¿äó~¢r[<¿ê_ý@²ø¿á'–
qH¿ïûÚ×Q‹
¿ï`낚y"UNASNone?ì%tA(?ÀĘtÖõ½?¾Ô_
÷&Â?ÀĘtÖõ¼?êòèÓ#M?ÎÃYÃ\օ?Lj4\³rÍ?ÎÃYÃ\ֆ?é\ ñ?´_Üçw‹¯?ˎ|;Óá?´_Üçw‹¯?ࢼ»à?¸˜ËYa'?Þº‡çòˆ??¸˜ËYa'4FGL J1934.2-1446?ä(_¼ B·À0!BoçÀ:ײãâ"À<]՞,¦@KßS75@ôK+w}?ա‰?ïúºEዡ@©¿f²¼€?òJ̌¶b?ïûÂ^ôÆ¿âI†[Ï¿âp&¾°ªW¿ïþª_ºz»?ïÁ5Ø)!¿ÛèFۆ£ôUNASNone?ï‡4t,"Ã?§ xGÉwJ?Ž2âôÚÏX?§ xGÉwJ?å8óeÄP?ÖI‰Ýö‹?Վ5âw`?ÖI‰Ýö‹?äÊy—fJÑ?µOsÙÄ?ÖkÑ3j^?µOsÙÄ?Ý5™ÿµç–?ÒCT·9?áe3%5?ÒCT·94FGL J1934.2+1036¿ïŸÔŒmÀdf±æÀ9ê¡/"À;q¨žð@u+'SO@êÓ²š?Î8×!qÍ?̪'».å?ûìÓi©@Ú!« §¿ç¼uÁù	A¿âŠI{õ¿ç«Úy]¹ï¿ç!¯}0­G¿ï÷ä]b0Í?ï(ڟsMUUNASNone?î¢0#±¦Z?¨ˆUµdF?¥ÜýÄåšh?¨ˆUµdF?ïEœQ¯ƒ×?±,Èø®Õ?—LuÊ…?±,Èø®Ö?æK¡|*+¢?¶•ü‹?m?Óh½«¨¼?¶•ü‹?m?îÒஊ»=?"­{"æ/ž?¢ÑõTL.?"­{"æ/ž4FGL J1935.0-0553?ØOnX"À(¾Ÿà·öÀ:(òvªHÀ;­Ëwb7-@^R 3Q;@Ç>
&Ê?ÌVïûÐñJ?ÉÀœþ('?û)¢á@ø@ÊQŠŒ5ƒ¿åu¿äF¼¿á"՝U漿êú©]\¿âSÓ¡Ó#ÿ¿ïÿÿ" 5•?ïâÞA>c¾UNASNone?)Ò
ß?¨àÃXnb?‰õ‹}HF?¨àÃXnb?飼?™'ƒP2t?…ø|U= :?™'ƒP2s?ëò(`"?±¹ÔÁ¢?Ãë¬7^}³?±¹ÔÁ¢?ï€N¦¦R?¢þ,f[?ìVVk|2?¢þ,fZ4FGL J1936.6+1921?ÎôÔÞCû¿è°IáÀ9"+zMÞÀ:µ®Ò­@Ù£‰²pÖ@€"Þ?ÉSàQäÏ"?Ì%=§*{Õ@àÌ¡-â'@Òÿ–ÎŽ?ٜ߯}‡?ïùRژg¿çÝgNòr¿æj}2…
¿ïþ;·f3?ï±<î×íUNASNone?Ê'âCÂs˜?ÅàÇͯ?évoc?ÅàÇͯ?×Êl_†º?Óká)P¸?äwÉÐ<¤?Óká)P¸?ÒZãÏfK?·*n‡e?æÒðLÛ?·*n‡e?È»Á™–Î?·9æíó?éÑ™šL?·9æíó4FGL J1937.1-0444¿é5K˜FµÀ(¥îÇÉXÀ:§
ûÅ<À;בÕùµ@ŽÊɽMÔ@Ñò¦{)l?ʞ#×u;?x	‰k¤ï?´!ˆ¬6@5™ ûb·?ïO5'‰ ¿ì¿ôÕ÷¿âѱkë¿âLERðgÝ¿ß=W´¿ï÷ˆ—é–1UNASNone?ïé
T£I?eT(–Ì!?fõ«\¶â?eT(–Ì ?ïøu`ùB?lgdƒ¸vŒ?N*}øüm?lgdƒ¸vŽ?ïL˜Ê¾?"p;Hú±?žl濈:?"p;Hú±?ïÉ&Bû¾?gÞdK¿µ¢?{lÞó Í?gÞdK¿µ¤4FGL J1939.7-1242¿³ä78+ÕÀ0`À½ÊÑJÀ:OL{ٕ2À;äñ"«=@ã7sá%@÷>^‡?Ï"/)ä*?ԏ=?{•ø@VÿëJ?òoðJÖ=?ïá·uL³7¿ã¬u:'Ä¿éb†ÝÕ2Í¿åãÈý4s¥¿ïÿÕ} i¿ïä×»=XPUNASNone?îVÌÇ4,~?²}xP'Ã?ª"3Œ½8$?²}xP'Ã?ç,ôe¸7S?ÓæÔEÃ%e?Ѧ4'Y?ÓæÔEÃ%e?çQqÜÙ¨ò?´È!9ÔG?Ñ]FL®?´È!9ÔG?Íj'Y¼d?°á4³º(?è¥[©þf?°á4³º(4FGL J1940.2-2511¿à¸û.ö;À5[«!ZÀ:61•¤A"À</Æ|P³w@Œ8ê8C@ZمAóÀ?¿ŒãÓ¤'V?ЀhûÂÄ@·»Ã
@%£fÌè¦?ïщàiÝ¿»Ž>Wå«¿ãi–!!Ë¿æö.Åæ(¾¿æåP¡F6¿ïÿÿ" 5•UNASNone?è@,B?ÄÖä'?ÏÓòÿN÷š?ÄÖä'?çÖ;Abèð?Ð!ŒQÐàT?ÐS‰}:. ?Ð!ŒQÐàT?æ¬U±2Ø?¸‡éú9Ë?ÓЧTšP?¸‡éú9Ì?èQõ"x-?¨ódÕtÆ?θ)ï¶N?¨ódÕtÆ4FGL J1943.9+2841?͛B­Êù@!‹zՉÀ:—{!ŽÀ;ú¨(÷@UÕ¢ß="?ÿ'þtå…*?ÒM£!Ø?á÷Ix@æþ*¼l?û?P"]?è¤zÏ)¿éS-Ú-Þ`¿Âë·sŸ4
¿å0>·ç¿ïûêAQÙç¿Þ»k›¯svUNASNone	?èbÉQòÕì?Æâ\Q?ÎtÚ¸4¨R?Æâ\Q?ßýù'Vîu?ÖY»¡e¸?à6ԈÅ?ÖY»¡e¸?╺Ÿ?½0©)o?ÚÕƋïÖÃ?½0©)o?ÚØîA(•Y?´ŒÓ"øK?ⓈßkµT?´ŒÓ"øK4FGL J1944.8+4301?Ã
Á‡áC³@"ˆ^	}À:ߝcRµ¯À<®nƒkYë@š7›Í¦?ûewS´?вï«ôæ?ÝßÉÿ'ò¶@
°Ð?Hl?ð\^š/A¿î'@"ªt?ïý%Ÿ÷¬Ÿ¿Ð×L¶8Œ¿·ByLG+c¿ë4rÞn೿ïÿþ½à ¿UNASNone3FGL J1944.8+4300?í<—Îœ\?´êV%'h?¶A‹m#?´êV%'g?Ȋÿ(˜ôæ?Ñ݃ߦ­m?éÝ@5ÙÂÇ?Ñ݃ߦ­m?àÚá‰ñÕÕ?¼U?ÞJ<ìTT?¼U?Á*ðß™?¨uX
Å?ëµC߈9Ù?¨uX
Å4FGL J1946.5-1527?îÕ}X:ÎÀ3ªCåÀ:­;qÆÀ<2©ˆúåå@+QœU@MdQ¹08?ÌZÂl½?ÖÂ{»[@û͆00I@$_6œIL?å*zAå}ž¿ØôKâ»'¿ÒЖ‰B¿ä¶ÌR֒¿íÈi[
lпïÚ/÷>_UNASNone?Ùtæü…fW?ʵ¦/†àÕ?ãEŒ½LÔ?ʵ¦/†àÕ?â½>ì:ü?Ó'É­ºZ?څ''‹â?Ó'É­ºZ?ÙÁHñ´?½‡Ìog?ã}[‡s¦?½‡Ìog?ã㏨ÿ?´fpRӖ?Ùé8à®?´fpRӖ4FGL J1947.0+0031¿á@–wfœ]À(2¦Òg@À;KÍ]ìÀ<±
À¾¢@Ͷ˃¡‹?þˆKBôqW?ѧ+='¨?ãŽYM= @º2nU"@ìé‰ò?ïõ-¿‰?ïý¤ Y?Ùς‰²›É¿Û®âÛ¬ä¿ê¬í3t¡"¿ïý4©Tø€UNASNone?éW["?Å~ůü°)?˪¡ÁŠ"y?Å~ůü°)?㌺ÿ¼À¾?ÕÄK¨Ïh?Ø抆~ƒ?ÕÄK¨Ïg?؃üFØ`?¸O'Õa÷?ã¾Ü÷Ñ?¸O'Õa÷?Ù½
-(B?»W3_£û¹?ãu!yikß?»W3_£û¹4FGL J1947.1+1729¿Ã˜•¤°OÀËEˆ MÀ:~]yWÚ²À;ïpx8 @YYJt@ˆÞ{Jùù?Ò¢É4<?à®
>¬ãù@&Á» ÒÞ@ªåq^?ëgÇÅ&^?ïÍýº¿Üê¥OÛ5¿ßŽØ'?Ù¿íÃÌ"'áÇ¿ïéý"ë´ïUNASNone?æÑß/>/?Ç1ÍJ1?ÓÀ\A¡ƒ¡?Ç1ÍJ1?êQèG;'?ÍùÍ­â",?Ƹ^ãaÃ?ÍùÍ­â",?åˆO»DŸ ?µõ«Îœy?Ôï`‰vÁÁ?µõ«Îœy?ã4µz-0Ë?¸2dï)©:?ٖ•¥žm?¸2dï)©:4FGL J1947.6-1121¿é­PÚE£À1'à°«À:&whiÏÀ;ñ"ï¾i]@LAô—2@÷T°[|þ?Àò1uÃÑ|?ËÚ\S=@áÝBeÖ@îa§ºÅ?îúA¯Í¸…¿äÅïbùÊ¿ä˜zJHùn¿ä¶"¡¸!¿í6A
çI¿ïÿï0l¯UNASNone3FGL J1947.4-1121?ÛS›åí{A?Ê_»XOñ?âV2
	B_?Ê_»XOò?ãHMð²¯í?ÒJâ‹`ê?Ùodš '?ÒJâ‹`ê?Þ±";R}?ºtzöNMl?àô'6bVÂ?ºtzöNMl?á°ç}wL)?±p´üâZl?ܞ1g®?±p´üâZl4FGL J1948.0-2845?ä¤Ñx½lÀ87÷ß (À:Âôí}F}À<'øxLAø@õÉ¬²@ÝӅM²:?Ҋä?Z2ü?ÆÍyÛc='?öéjâÌéR@vMP¦?ïó÷H¡Y¿èM!@—tÑ¿Þwgà¹é›¿åá*È*§¿ð¿ïýl§ÉEUNASNone?ïðÓ|2þ?i'q'~ù?^Y›Ò7?i'q'~ú?ïÎ`¡ÚEÌ?°ê£à?xϯÝc?°ê£á?íà¡G<{—? ;–Ÿñ­?°úõÆ#M? ;–Ÿñ¬?ïHF9
'¼?ºö5Ñ?–÷8ÞO¨Y?ºö5Ð4FGL J1948.1+2511?ÕT÷Ë	06¿ÆÆ»üXÀ: !}(IËÀ;ÎôX,@ŸR–$ð@L¦¼—Ëc?Õ¶?!}ÿ	?ïý½À•[ò@Ö|^p@'ܾ²X¿îêÎà£Cg?ïƒP˜È¹¿ÂTR½'M¿îAŸÀäa¿åË@¥â}8¿ïþ½_ÇeÛUNASNone?ä@°'0ë?ÎB'G¥Vj?×~žûž)õ?ÎB'G¥Vk?þ3…Á³º?ΊQ/@ùx?ës"?ΊQ/@ùx?áÍDÇb?¸6ÐéÊ+Ë?Ýùúevq:?¸6ÐéÊ+Ë?ÅrbuÕcÅ?±bÒG­½?ê£gbŠ§?±bÒG­¼4FGL J1948.9+3414?í‡óçcf@ùÉÕ¡‡¥À:Œ%ÿnÀ<d._ŽÛÐ@€Pþ .‰@'ƒ$ã?Ì)FNm÷?ã$"¯&ɘ@4·|Ùor@*¥"8äù¿ïþ1ɦ§Ÿ?ïÚÚ¬‰`f¿Ï®öxçù¿á©=¦~¯¿ïÿ›‹â ò?×Fë¡Ï4UNASNone?Ê\xÿà?ÄPtPFº?éháÀ8ú?ÄPtPF»?Ųå¦K?ÏYÞ.>ð¼?껓z†–n?ÏYÞ.>ð¾?ÀîRO?ª¹¥9Èm?ëÄkyl9ú?ª¹¥9Èk?Ø´pGù<%?ºàf"öŠ'?ã¥ÇÜaî?ºàf"öŠ'4FGL J1949.2-1453?ë
ÔåÜraÀ3c 1ί%À:9ìTRÀ< 5)­x@584¤ÍT@º®ƒ?Â-æ˜$ú`?Ïç™Â3k½@
®Æ±@£'ôf™½¿çXJCðñ¿Ö·_þs¿ã
çŸïõ¿ã9>Js¿ï¾'€p}Á¿ïûúëÄ	UNASNone3FGL J1949.5-1454?Í6/÷6¤?ÃPšêÆ°J?è²t2W?ÃPšêÆ°I?â^›"ɼ?Ó"ŠëðA?ÛBÈØl‡Ø?Ó"ŠëðA?ÓÿþÉ{"?¸~9üfx"?æ›Bnö?¸~9üfx'?á^ÀlBÝ?¸¾	¾ßã½?ÝýB'zF?¸¾	¾ßã½4FGL J1951.0+2523?è:ÜÀwkʿ俎‹HÿÀ9á8ˆÝ‰³À;‰á<ÆYì@\fHß@´±'Äjþ?ЅÁ?ÐÐh?èlŠlÕì@ûà\÷R@½çMVŸõ?ïðäÚ	Ì2¿ßöP<Xv¿Ó&íàBËW¿ê»Á¬Þü¿î*GÒ&©¿ïü UŠ÷UNASNone	?¡mLÙx3?£wü¡vÝ?îé.›2h}?£wü¡vÝ?½²¨ú.Š?ʇ!=?ìIªàº.¿?ʇ!=?´°Õ­!?¡ˆ¦Ÿ ?í}©åJ]{?¡ˆ¦Ÿ ?˜Šc‹[õ?€iò&oWÛ?ï;¬çó¥!?€iò&oWÛ4FGL J1951.3-8015c?í2ˆ?—À=;0aǛ5À:P,á	š³À;þí¢/jQ@p*^£N@(ô€oüè?Îå?	U>?ÉsN@Õ³%?ùи´çÓ¹@Ù1΄1þ¿è"Xº¬8Ù¿ÞNvZ¥=¿äÂAƒ-¿çÜzŸƒh€¿ïü»ýǖ'¿îì:ñm–UNASNone ?ïlÒ~RG?•Z%z@ ?'e°5·
î?•Z%z@!?ïÁ½ˆ¨"Ë?•®¾–"x?!;«µšU?•®¾–"y?ëñå6v¼?¯³y½Ø´û?Ø8k&%?¯³y½Ø´û?ï`¿!?Šäò¤f)?Óè{Ð?Šäò¤f)4FGL J1951.6+2621?ï{ÃRÍ¿ÑTËß<'À9=kŠ'•™À:ÉV¸syt@‹ž[JS‹@ÓQùÇכ?ÅÔ\c-L?ÑÀª?.>,@U-úNw@#^邏?ê_åBåWÞ?ï–Ï)ž_¿âcž\vù¿ëN
>¬ãù¿çüÎR
¿ç`oâ*ðUNASNone?¶¿J©¾y?º¦-.|•?í/ȪÈ1?º¦-.|•?²Tò4pj?À"Xo¸®?íµ~!¹qó?À"Xo¸®?и¥"	'Û?´‡@'áw?磭6{>'?´‡@'áw?®†žÆ¬)?žA¯Õg!?•=?žA¯Õg!4FGL J1953.5+3841?ƒë£Ä¬ƒ@¾Ès«ÉÀ9"w3"«À;Á15,2@¾á˜5ìK@žŠdrp`?¿ÈYök®?ĽßwŸI?þEÀi;'@;1KýYˆ¿íª¬çT7?ïô"&"À¿æ¬Žhãï(¿ã¢»a—è¿ëVœ_˜¿Ö1q<-WÒUNASNone3FGL J1953.3+3847?æQ¾Ñ1+¿?ÌhMåōZ?Ó\']¨?ÌhMåōZ?쭄A':²?ÅuOUò7?º"ÝöÆ*o?ÅuOUò7?èéR's?¸¬["ó=?ÌZ·…ö3š?¸¬["ó=?쓃ӕÊã?§")'ÝG?»cácQ¨é?§")'ÝH4FGL J1954.4-3729¿îQœ« ýÀ;û¨`ܹªÀ:Æ(¯K²†À<=b†ž@åXvc´…@áhšô­?ÒùYÞÍÒ?Ð
Èâ¬?õð ŽëÁ@±:ªËÆ¿ì Ð?Hl?»Ã!¨FZ­¿âMUô([i¿äy^½zŸ¿ïëÆ!·à¬¿ï"ÝíÜgUNASNone?ïÔÞöQô=?z¶J#ö«?u"×á–?z¶J#öª?ïùíÃ
?pKÏKÇÞ?HK˜óËÖÉ?pKÏKÇÞ?í¬¾‹˜i? ñØ¢?²š£<·? ñØ¢?ï¿áŒ€é?pûTÌô?€»ßŲ?pûTÌô4FGL J1954.5+2420?×:Jü÷°¿ýäH•:À:0S5À;¥Ã<*Rº@Ð3öýwå@L¢À‰Èk?ÓZe¼Tº?äòSÍÝn@à:2*õw@÷l¿›áÈ?ïþ
¡ÿϿ㠝™ÙZ¿ÖÈhûí¿è­µ°P•¿ï÷!ŸŒø¡¿ïë	εÛUNASNone?êϒ8¶WN?ā/>OW?ÄÁ·&¢Æ?ā/>OW?ã	uoУ?ÔûÎùšÀ~?Ùí _ܺ?ÔûÎùšÀ~?Ø«"hö#?º7a/óÀt?ãªn˄ñð?º7a/óÀt?Þ å‡ÿ¼?´ë‹ö:L?àò¯<!?´ë‹ö:L4FGL J1954.8+2543c?ïÿÒ¸–¿ó4(%¸÷À9Q,?#+~À:Ù­´Ù'@
O$«[
@œãÞaIÇ?˧tù|-M?ÖK^£#†@JO‡&ÐN@Õuèºi?ï袠ÿ>?îFâ< š?¿ê¦WþÊ&¿çl1aKõL¿ïñ½m捿á
qs	âØUNASNone1?ғʾI"?͜j§8ò£?æ¶ð Û=?͜j§8ò£?ÁÌÖØ#ÓH?ÊúB}éU?ëŒÊI÷.?ÊúB}éU?Ò#šª¶Cs?³‡mZò{Ç?æî2ª¤ÞG?³‡mZò{Ç?ž—¼2ß}?¡+m·`l?ïGri?¡+m·`k4FGL J1955.3-5032¿ê&&ÝVÀ>'àãF·À:ÀöÞN«À<r¦Q8ø@bü}"€U@ø½=ã^?¹÷(€|½¿·vœ¿há?þ{ÓJ•Oˆ@>•=im¿ãëÙ7>Z¯¿ä[ÇqC9;¿è"ÏöLø׿䦰~ L¿á¬ïícEJ¿ÊNC"å¢UNASNone?ïû ö>Q?E.+Ó¿D¼?C|'â¾%?E.+Ó¿D½?ïü5\É?i+t\ס?>S}º ?i+t\ס?ïքûååÈ?w,á߀;?t½'

7?w,á߀:?ïñ½ÜȨ'?MUsDÍ­Ù?\"Fn®úü?MUsDÍ­Ú4FGL J1955.8-1657?æÀ5À5¨ßXÀ‹vÀ:i1òÁSÀ;õͧ¾‹@+ÌAaŸ,@\…×Dö?Åy£¯ò÷?OÁ—ËŸak?û€©E5?Û&¸{‡	õ?×wEÜ®S¿éDÔ`?ù¿éhšô¬·¿çÉc‹À"?ᐣñâ0UNASNone?ïfUU1?•(ñûV?"=¿ÕUYÁ?•(ñûV?ï¡Ìî­Z;?›þ-Å3
?‡ŒÄT©q4?›þ-Å3?î=¢?^?™š¿Þ9L?¬%Ü®Ú?™š¿Þ9M?ï5j³OÝÍ?ˆM®.g¨?™R©–F\?ˆM®.g©4FGL J1955.8+1154?ææIˆ^vÀ ôuĨ;À;Ž"ÝÀ=óí£*@ "µ$¨?þNÚ"ö¥
?ÛFqÏsÆ?ïn>Â2"þ@߃ê?þ÷öüK@?ÒÖÊ|tW¿ïÿëJw?ïýš)âQ™?Á» <‹v–¿ìÞzt¿ïýSG¥°ÿUNASNone?ë 5úX[?¾|±
5ñ?Ã(ž"ò?¾|±
5ò?á'ãÐd×y?×P±³Í?ÜÚ8_6Q?×P±³Î?éî쎺?²L{öE¢?Èó¥DMÅ?²L{öE¢?Õôcúå?Ãù)ÒÜÛú?åôο?Ãù)ÒÜÛú4FGL J1956.6-7011?¯¦ýo'aÀ>ç¶þ.n¨À;™÷
ø|À=V%Ýà‡@((ú@@«~žk?ÔÄ_`7Î#?ïÿäâBTä@ÜR¾éµ;@("nmØ?ÓڞF§"¿äëgø6Ýã?âËà=ÂÙ¿àhK_·K¿ïÿd†'V?áécÜHkUNASNone?Önç=®?Ðö˜A×Ü´?äȌa?s)?Ðö˜A×ܵ?ݽ7Œ!‰?Ö6H¢÷d?á!d9ï|;?Ö6H¢÷d?×hð–6§V?¼.D˜Î?äK‡´ä¬U?¼.D˜Î?ÑËEdŒg?½}¥~;?çwš]M¹Ì?½}¥~;4FGL J1957.6+1230?ª§£ÂmÜ2À!_€™"À:ˆ·m¿öûÀ< d©ÍÄD@d'8Ôþ?ÿ'ØÚø	?Ѽ
éÿ
?ÓÄcœ²}Á@ÕÖ¾¾Q@».\^Ñ¿ïß#FV%§?ë[–©û¿ÓN­âü¹ú¿ã¥*&D7g¿âþP§ET¿ïÿýawUNASNone?ï'Ý[õn˜?xæAŠý?‹H©¤Yô?xæAŠý?ïË.™o‡-?'ÂÖã
–?zh³H<i{?'ÂÖã
–?ëßNԕGš?«(Ø;"??À'Ä­ªá˜?«(Ø;"??îXhçç"?'?çzyÐ(?ªyqŽÁ?'?çzyÐ(4FGL J1959.3-6121¿éà[®oÀ?¦bfýeÀ;¢™=SHÀ<êI"Çȁ@!VH‹´ÿ|?ò+ŽXó·?ã8b1?í'ѹ›—¡@N»Ÿ}ß)@\ƒÐ`«¿ïÿÓõµú"?ï÷AJM+,¿È=a	…:?æ"Ñá^ª/¿âQ'W«¸€¿áÃÙDr UNASNone?ïó®ïø¬Ç?Y?#ô™?X¢ ¦r¬?Y?#ôž?ïø9h'©ô?pn'.ÓÞÖ?O]µX2î?pn'.ÓÞÔ?ïl%Ú\!³?‹?øË3™ü?'{D´{ɯ?‹?øË3™ÿ?ïÑm6¬uƒ?s#Š†MØ´?wId©Å>†?s#Š†MØ´4FGL J1959.9-4605?µ¡öû¯¥JÀ>­ú‡;À;ßúTÅT3À<푮éŒ÷@"Y:-ù8?óxÏÞ±Ò?à´/è%ç?Ù¯Üüð¬?÷Ì_‰ÓRù@}%
«:¿îØúØxÒ?ﳬ ›%¿íç^~:˜'?ÉWw¬	?½ y1Å¿áŸê¶ÂŸLUNASNone?ï÷'ç˜F?Q¨c67cŸ?Pú0ÏsÞ6?Q¨c67c ?ïýÏށDé?QÿH®M3]?1õز?QÿH®M3Z?ïºÏ¤_r3?~'g"÷´¤?Lè#rù?~'g"÷´¡?ïüƒ,€Ë?8þ¡'¨Ý?;çV›ù­'?8þ¡'¨Üý4FGL J1959.9+1833?çû›qV7À¼Pbîâ¡À:|³_=}9À;ç¶jŠ¸U@æ"Ôei@™íeÊ?ÏMò?Ò³×Ùõ@Ëi¥¶Ž?û•P9(j­?ïýà€ˆÑu¿æG¡Ÿw¿á·T*#¿ù¿àÑNÂò®¿ïýZØ®¿ïýl<i<ÚUNASNone?îˆËyÇ#?®eÄý¨"?§sHcÎ–?®eÄý¨"?ë'ÐiòÆ?È£%ÐB?Ã`¾X4çò?È£%ÐB?å¨ïLUå?µÔ¶üLò4?Ô®!gT5å?µÔ¶üLò4?á÷ÌC×p.?´?¶Æ"´?ÜgxQ¥?´?¶Æ"³4FGL J2001.5+1611?ÝôÍO€,iÀñ¾±ìÀ:ÞkZÁíÀ;Շºtµ@ý-Ûö@Æw}åÞí?ÐR—\R'G?ÛS%âØp@(Ëwb?ùqoXþHñ?ãwÁm9Í¿ààM³9ä¿é	(Ó]à†¿ènn¨TG€¿è±òá‰rZ¿ïÿô╋îUNASNone?çº/óÕ?È©†°½?ЋŠèU?È©†°½?åý´‹<w?Ҕ;E3Îì?Ô–é‡ç?Ҕ;E3Îì?á¥DsŠÑ\?¸MþÓՅ?ܵwê]F?¸MþÓՅ?ÔadW/¶?³¼!#ÐÌ?åÏMúTh&?³¼!#ÐÌ4FGL J2001.5-0958?íñ|1ÛÖÀ4ß«÷jÀ:•GûATÀ<ÝË!Ñâ@QaÒ-ø@â
Üa•F?Ó'½ÝEÁ?ÃU´'Œ¶?òÖ0=µm5?ù(ï7…Ó?ïšúAп睨ÇßÓ¿ëý7Þ¾'Ì¿åÚKäÚá¿ëY*GÒ'?Î}šàkUNASNone?ï3]8.›?ŸËµ}ÚM`?™"^xú,¸?ŸËµ}ÚM`?íôijžË?»u3Þ?°YÚc	§{?»u3Þ?ìÑ­Ô¥»ß?¥QÓYê"?¹r'ZÒ!?¥QÓYê"?êÃþ>C?¬õ"£cÁ?Äð¿¿÷?¬õ"£cÁ4FGL J2005.8+3357¿Ù«;0Ou­?ñxE܃#6À9VÆÀCQŽÀ:›tkâ§*@ >vx'GÃ@ãÕº²?ÁYɟñ¢o¿¨-;¼2Ž?ð%ôkwG_@ö§uzU‡¿î
9	6	§?ïí֝0'¿çÕ¹€ቿë9ÝaD"ƒ¿èïî:ß?Ŕrþ¥7UNASNone?íeœ'ùc=?ºh"@䓂?´Óh4æ?ºh"@䓂?ìðœoßX–?ÉZ­,®˜>?¸{;T?ÉZ­,®˜>?é)]'–P5?¸œÓX>²?ËZ‹a¦¿.?¸œÓX>²?ï.S_—?'G¿é§â¨?š5Ÿô
®?'G¿é§â¨4FGL J2006.0-6538¿êôôx|±À@ï$©ÁÀ<©1½nÀ=¬tg°é@#'ó‡÷†?÷%ˆ»%œ?â}Ÿ"Ò?Êb¯ã Ü?îÓ·¢™œ?ô qÇîk®¿ïZu%F¿ïö†5•8?ð¿Ó½SG¥°ÿ¿åËJÍǟ?Ðmû½ñhUNASNone?ïüõ‹j/?:'zy´5ñ?8S¤®‡?:'zy´6?ïô9u÷\?}âÞ¹àø?WÚG?}âÞ¹àù?ïT@béÙ¦?'ðmâ×T?•wó¢ÄË3?'ðmâ×U?'`Q[?€´J]řÖ?ˆ6'ë©O?€´J]řÖ4FGL J2006.4-0354?íbˆ¬ïÀ2v…¹èÄzÀ:àUӌÚÀ<'ÅÅqŽ¹@›,™f
@a
;Ã$­?ÉyD$>û?•P?J£?ÏôÔ¾2Ö@þv·Au@?¤–á?æ°§2È¿é¬"qÌ¿æq²à<–3¿ÄïXgö…¿ïóqal+¢UNASNone?ïêRήl`?i1iœP?e­1Q"ž–?i1iœP?ïüƒãEõ-?aÁ¡¾I['?;àåÐV•?aÁ¡¾I[~?ï]ÚM¿8¸?œ¢6Vc?"D¶Hé?œ¢6Vb?ïêˬm?X«'ݲw?e4÷üS"ì?X«'ݲo4FGL J2006.4+1834¿'ñ6a=®ÀýۘAªÅÀ;'~B%>À<Xæk"@ òc'?ýlÖÂïÔ?Öô¢Ô«¾_?Êö²¤W±?ùŽ"î9.@–Ѿ#<¿à O–@I?ïñQçS`пíî+÷Տ?ã_ïSàR¿äËôï#¿ç×Fm¢šÊUNASNone?ïúâȇB?I'oO/µq?GŒtÝâø´?I'oO/µm?ï÷\ÉÁ?"0'™¾M?QFl|ÅӃ?"0'™¾L?ïh\ßC?{{GAmÉ?'ômäŸ×?{{GAmÌ?ïçW-+ÿ?a•õ".b?h¨úÒÔH?a•õ".`4FGL J2007.0+0707¿Ü?N I»âÀ*"œ
!¼À:2wKøÀ;ðK+w}@`Õ²yc@YOýnUH?ÉÃ]wÕN§?®¿»ŸÜ\j?å:áqÊ@҉SP_¿å$ô,¿æ6¢ôŒ.w¿äþö€$}Ž¿çiqÛ¯¿àîç©Çå¿ïÿóÖ&ãUNASNone?ïò¤Ý‡2?V'_ØUR?Z¶Dñ›ó¨?V'_ØUP?ïöŸ…0î´?rÀDRùI?RÀõž"•J?rÀDRùI?ïIààh‹?-+益?–Ç‹ãòî"?-+瘟?ïʃŸØ´ú?hæùGÏ?z¾0¥ƒ?hæùGÏ4FGL J2007.2-3157¿ï:Ô.ºÙ¤À=1ðÃLÀ:=ƒá¡pÀ<<Ãþ¬C@+,õVƒÅ@¡|å-ì¢?Äaºö¶€?È´ÃÁ‹P+@¨³Ûd?E?ïuo]þ/?îגŽ¿Â4]ë¿ÝôÑc4'¿¿âŸ……`ý¿é¤IöÄ¿ïâòÞ¯M`UNASNone?蚹‡É>:?ÄtÖz&³?͕àÛ?ÄtÖz&³?çT"{ˆjl?Ó¹L½ÏÖ?ÑV×ï+)?Ó¹L½Ï×?éªîOæƜ?²…o ˆ?ÉTFÀdå'?²…o ˆ?Ï·IO²¿Ñ?®Z³'wÆ
?è-¬P?®Z³'wÆ
4FGL J2007.9+2511?ÛÙÂ7<'ÀÌ W"ýÀ:Vã®À;Úà!p"@ŒÛâêE"@Â&ޑo?Ëk›¦ÿ?áqðþZcy@•ÚÈ8?ìÙAéj£s?ïÿs}¦¿Ñ¥!øxLB¿š…}`††¿ä'á4¸Ä¿ë=3g5™?¿ëëԚ ¨UNASNone?ÊJÓ«¾;?Ë;KOú^?ém}q?Ë;KOú_?Ñáàû?ÓšÓi=?çzü¸?ÓšÓi=?Ä#äÁ£l?°‹)Úam?ê÷ϗ?d?°‹)Úam?unj§ªT?`¥Tª€®Î?ïÕé#*°¬?`¥Tª€®Î4FGL J2008.4+1619?ïÛð4#¢ôÀ!§"š|©À:ÐI!²oÀ<Aٌίü@ {3§ø,?Ñô{<ŒMV?âÛ ö¼Š?ïÝÊì!üª?ûº£º"ˬ@¨[#*¿Ý]pH'¿ì9)í9Sß¿æîá(úJ?µîÓTPd¿áÆsxŠ¿ïÿþøþ"UNASNone?ïü5†{¦?Fð´˜"¦?>SƒÌ"Íì?Fð´˜"¢?ïüñÂß?kË`…w¬3?8w'ùéu?kË`…w¬3?îÿÍÈDoZ?•â²ù\H­? #{¹
a?•â²ù\H¬?ïûm± ½o?Câ©b¥?BI;}
Gé?Câ©b¥4FGL J2009.5+2425?é1«òC³Àïdþ‡YüÀ:Šh¤.HÀ;hFDe@cÉÑÅ°@§ÛðuI?Òò)=;å?ÜA^#÷«ô@äàTi
á?Üϧº'i?ïþr–öQ+¿×æÓs¯û¿ç=¥b$¸F¿ìŽpK™\¿ïÿ']<9¿í·ØIёUNASNone	?뚣¿&?ÇÙâ+,¹¦?Á—áqeÍ?ÇÙâ+,¹¨?ÚÜAV'Ä7?׆üÁ@TÑ?â'ßT·ä?׆üÁ@TÑ?×#¶­´‰Á?·–ß$"N?än$©%» ?·–ß$"M?XÌÀôüe?FJ´bÿ´?ï󙟅ø?FJ´bÿ´4FGL J2009.9-2116¿é#
"Aí|À:ZA€ÓÏöÀ;	±oy4ŸÀ<ÎÛÈRé@àµFsW?ý…Á•a&?ÎMúI\ÀJ?ãÃBàO`@´Õ½6VÔ?üæÒâ¿ï'¡­º8?ïþo§WÈ>?Õ-•d€³¿ãb:[€Y¿êÇ
H½ß¿ïÿ²2ӁUNASNone3FGL J2010.0-2120?ÓöŠX­ðê?ƒJíKξ?æºÓ©‹?ƒJíKξ?ÔÏNçŒË?Òð8Ú?å˜XŒ9ñš?Òð8Ú?É«Rûï$Å?±ëóªƒ)?é•+A6Ï?±ëóªƒ(?È+÷}ȵ?­šÇS1uó?éõ ¹Ó?­šÇS1uô4FGL J2012.1-5234?í£Þk'À@£}é9êÝÀ;CšMô€À<¢È£r`p@"¨YßDs¢?üé
	Ó¾Y?¸éú=|b¿ÀJNØ«'a@ñÿ ÜïZ?òà-"ã§Z¿êiU./¾4¿ãºßr#¿ìyÄaÄ@6?ÞpØûYR,¿é,Žž"Ô^?Ð;e[Ï_UNASNone?ïú[#¸'´?G9º6/?F"qµ1í?G9º6,?îC	Eî?Áì^QV|?«Ïk£Å?Áì^QV|?ï:ôhyÜ6?'´¨ø̺G?˜¡rðÄy&?'´¨ø̺H?î1ªZʙ?¦… uÑ?¬å^ÊSVq?¦… uÐ4FGL J2013.9-8717¿ÞS6'"«²À<°_®¼À;¤'[rÏÀ<֑¹ÑG†@!29OWB?÷4Œê^®?Ù=œ˜§?Ø}jŽê/?þw'Þ"um?úàï""n¿ïýxÑ¢õc¿ÝñïÜqZ‹?ì÷ª%Øם?²<£Ip·M¿×6‹{U6¿èŽá¯²áUNASNone?ïøîZ.V?I…wÄå8D?OèF—F¨x?I…wÄå8F?ïúˆµMÑþ?iRªuù]?EÝ*ȸh?iRªuù\?ï R'·ª?…Ó¯	>Ú?‡ükv"?…Ó¯	>Ú?ïÑ"n¼+Â?i-ü'?wnÈ¡ê??i-ü"4FGL J2014.9+1225¿ë»rkì!íÀ(n$ÛÀ:¬%¦'¶(À<rÛ¿®×@'}‹qÞ@|Zœ-Ȑ?É¥>}êª?¨ÙMþTs?àá¡Au@Uzæ{¯¿îxx¢(3{?³/ÈðtFÏ¿ë[iw'ß¿Ï*ö´Ò°¿ãê–vÏj6¿ðUNASNone?ïïŸ8•,ü?h<ªtȬ?``ÇjÓø?h<ªtÈ®?ïù×â¦?j.Ì1p!?H wg"?j.Ì1p!?îèx$Ò?–Iöšt—!?¡x}¿òߏ?–Iöšt—!?ïæ8Š‡m?['!Bî?iÇux'ì!?['!Bå4FGL J2015.3+0758?ïmœݚAÀ-:}ªOÊCÀ:hꭈcçÀ;ÙRé±ßá@…xÐK\u@üô}þ•?¿å[9ºH¿²Ûae¿c?ów¨Èá…Á?ü³…ü-ãh?éà"¾ŽE©¿êûêâa‰ˆ¿å2d×.¿ê÷Ü_ïT¿ïò³±rÔ3?ïҌ)nŽSUNASNone?ïî´IFcK?dŽ67{?aK¶¹œµ³?dŽ67{?î×ÕHs'á?±É¾T)æ?¢'«x́ð?±É¾T)æ?î0Q2¥?Í°8*ê?¬ÿŠîœÕ¬?Í°8*ê	?îmXq²R?šY9Ý©8?©.êxäÚÙ?šY9Ý©84FGL J2017.3+3525¿Ê&ÈÆé|—¿´u"–ØÊÀ:Ç>A".ÎÀ<)I`œ"@!½Hö>
?ò_æ¤ì´?Øu\"•¬?ïÿïÚê@
É?äò]€?ü(^Η}5¿ëÖ?rÖÚ¿ì| ·Ûy¿Ò]
øGv?Ëz£_@,k¿åê{3}¿ïÿ~?ËòÝUNASNone?ìò¹ûƒœ?¶o5ŽâÁ?¸j0#ç'?¶o5ŽâÁ?ãÌaY'ÄÂ?Ø)D€ôl?Øg=M°v}?Ø)D€ôl?êO™–]T?°(Á=îyÆ?ÆÁ›µ¦Š°?°(Á=îyÆ?äíu®çq?ÁùçÃ×f?Ö%¢1è?ÁùçÃ×f4FGL J2017.9-0114¿Ø#8 ìù8À3¼î9.÷À;öÜjςÀ<[ƒ°úo@ræ@fU@
%ó¯?ÓsŽ!ì8ù?àèS¦pA±@ÚcÞÌ©'@§æž!ê¿ë>L×I''?î‡óÿÁ–¹¿×ó{B¤,¿èš† @¿ïüð§12¿ðUNASNone?ítûm¢?¶µ3I:Á?´X$'ï×?¶µ3I:Á?å"Æ_Ó\?Ñß×è‡"?ÕºsÏ@YH?Ñß×è‡"?æ(‹ãBI?³×£‡ø—?Ó¯þè9{p?³×£‡ø—?Þôý±½g×?¹BrŠ?à…'!L?¹BrŠ4FGL J2018.0+7903?׏ݟ§Íó@6©˜áõ²À;É+ml%À=Kh;R¼e@þµFÉ= @lñ<îØ?Õ×Ä3êé?ï&p­F@P¨>x
Ô@p£V0ä?Ô_2€ó¿×dŸg™¿¯Ó.±Í¿èélÀ"{¿ïÿàöO}¿ïþ€Ǒ$UNASNone?ߋ9×Èeh?Аq˜CÔ?à:cÍL?Аq˜CÔ?ÓœmIÖw?ÒÍS²*Ä?æu1É[Å?ÒÍS²*Ä?âI²öòË?¼=^=ñùó?Úálši?¼=^=ñùô?Çu‹¢]ü?«'Ó¾‹:?ê"~¨'?«'Ó¾‹94FGL J2019.6+0616?ÙݎbJ©zÀ0cÛ]‰HÀ:žcʪ³À;Ûxâií@ã`"jZ½@8ââ¸Ç\?η:ë
€?¿@1ôCß?óµý˜F³C@Ún9™~¿^£úF?ïõŸI[ê¿æ"@ ×f¿ê}ó¶E¡Ë¿æª§=Ç
ì¿Ê£]½ _UNASNone?ï¡6¡-Â?ˆø Èq?‡²W´¼O…?ˆø Èp?ï¤ñ<aÅ\?8œôMÌ?†Ã°çŽ©?8œôMË?í£"Î'T?£·#?p"·?²ãaŽÅd?£·#?p"·?îÛ»ãj#w?''¾°?¢DAÉ]Ș?''¾°4FGL J2021.9+3609?éʎ`¿Û5L½j¯À;hÙÞ-GÀ<
Ž7eÇÛ@$‰ç˜ã?éà§_ªài?âÛþCx?ïÿH è@uúX S?üJÓlN2¿ïûš?±Æ·?îJùÞ}Ï9¿ÕÒ½<64¿ïú²]à°Ú?ïåe¶™…?Âw´ÂiòbUNASNone?︣ñ½D?¢z§‹ÇÖï?×œ¯?¢z§‹ÇÖï?é½Í~??ÕՏЀ?ÉÊ·ó?ÕՏЀ?ê ðý?¬­Á-Ð ?ÇŒ<ó¥
?¬­Á-Ð €?ì"á˜Ã?¿þi`Eç?»`ó9çÇ!?¿þi`Eç4FGL J2023.3-1947?áè€XoКÀ<ÅAÈ!laÀ:Gû'½À<:»9&';@YžP7¥ß@óõÞ>Y?ÅI©Äå?Ä1s*.$?ûL¹ìö8?üþS¶‹¿ÜÅ3ü0耿åóû_‡O¿æ"f"?=¿ç>¸Ø#B$¿ïÿ*LÚ¤&¿êá'V¯UNASNone?ï"ùBœÄ"?Ÿ}vm1Ó¯?› ×¬g{Ú?Ÿ}vm1Ó¯?î܊["Uî?°E´'?¢7ZFÊ¡9?°E´'?îúaŸa?¡8VA•3)?®€Yæùò?¡8VA•3(?ìd!+q˜?¦>ŽL×Jí?¿ÌÞö¤s??¦>ŽL×Jí4FGL J2024.2+3616?î¦Ánðœ¿ç¿û}º@À9¼L¼ƒ©À:ÊèïBB›@ ¸dÁÅ@XÕ[ç‡c?Ð5†?º•òpw¿?ï¨E™gD³@
,€ÛÞ¿ïù}Ðwl?ïþR€ÖT5¿âß̃ѱ8¿ãV¶Zš€I¿éÆyÌt¸9¿àEa3 ¿UNASNone?ì%J
6í?Áf2)xÊî?¾Õ¯g–Hœ?Áf2)xÊî?éA<ÜX?Ót#Ñ!âÏ?ÊûÇ莠?Ót#Ñ!âÏ?æÊÈïª&‹?¼«îPÍ`?Òjn «²é?¼«îPÍ`?ì–s{¨þ?®ŠÔÎÔ÷ß?»Ld"¿?®ŠÔÎÔ÷Þ4FGL J2026.0+4718¿ì8H^!j—@^ÂRˆÀ:Ót«£‡YÀ<n´Ý¾V@ø²m¥õÈ?ÿ-5Ã0kÙ?Ӄ_èÈ×?æZË]a'@WgZ',–@²³HÂ;¤¿ïÿÒH6Ðw?ïìrº1¿–¿¥äká
؇¿ÒHSUèiá¿î1"áHÚº¿ïÕFƒrèUNASNone3FGL J2026.4+4709?æÐÊ#åÖK?Ä9Y–‰?Ò^k¸4Si?Ä9Y–‰?ÙG9]¢€y?Õ¤½I{¨S?ã\cQ.¿Ä?Õ¤½I{¨S?äªoŠÐœ?¹éøëìm‹?Ö«!þê^É?¹éøëìm?Ú,Ãsn­?¸!>~ÿ?âòéžFHª?¸!>~ÿ4FGL J2026.3+1431?çö|ÏÀ*ãjËGÀ:ËSïk]FÀ<«[ï@ôÙ4ª,?ú•çéóN?Ïȅ?o'?â=>»&²@‰`ÈW?þ§^3$k¿ï쾤ëÝ3?ï{ÆKç_¿·¾t¶¿×»o! ä'¿ëko"óh¿ïþÉA‰UNASNone3FGL J2026.3+1430?Ø$Y{Ã?É#ñoª?ãíüS}Â?É#ñoª?Ò$Ó;xÜ
?Ô," ƒŠ?æí–bC'ü?Ô," ƒ‰?Ï\ýƒËõP?µDv³Îh&?è(ÀŸ
­?µDv³Îh%?ҙ²'Æ=…?¶µ" Úý?æ³&¶œá=?¶µ" Úý4FGL J2027.0+2811?ɵpÀ‡oó­â&À9¬ŠS«x¿À<©"àß@Ans{!ß@z*ž9;‹?Á *†<ð?ë7ZU¶ì@!ýAØèd@YøŠ•Æ?ïû/²?¶Âa C?¿Ü7e\{+¿íô×x!yÍ¿ï÷M@ÝÁ¿ïÎ߁Z]šUNASNone3FGL J2026.8+2813?¯fŠ'?¸¢èrígÍ?îN9—Vþ?¸¢èrígÌ?'<Ô.§þ?‰`­Bh?ï·¯óE`?‰`­Bh?µ¿¥äQV?¦,l>Ñ?íHCuÝv?¦,l>Ñ?JûxN'³"?9Í&ZK¿?ïùA!ì[T?9Í&ZK¿4FGL J2029.1-3050?îìܚnÀ@­
A1"¸À:¬\qðÞ$À<6.#)@"Pðˆi@P9Ô7$?Ñ9¾½•wK?ÊûW2'?õ¬8Ï
@öåS+v%¿¸K"@'ý¿æâCÏb©¿éÍÕáH"Ô¿ätáÙú2¿ïÿŠ#ÚМ?¦¡€Ã´ËUNASNone?ïóL÷U¾7?^£èpÜÅB?YfTƒ²?^£èpÜÅ??ïÒkU7Õ?Œñ"*
]?vòJUdb?Œñ"*
^?îFƒ¹ ?œ¥Ñ÷Ÿ'^?«žÿÇÄeú?œ¥Ñ÷Ÿ'^?ïË&'Ôˆh?jHÙӖŠ?zl·»Ì+?jHÙӖ4FGL J2029.4+1013¿ë9ãш;À0dô¥Xê}À:Œ^×ü«¸À;ï&<ª«:@÷\1X$@Ìa¢—o?Ý$‡¾û¨Ø?ÛjŸ(Ï­?òÓ<7¾³/?ø"ãäës·ˆ¿ê"k'Qտᡚÿöø¿èLewS¿ïúý—oó®?ï€Ú…óUNASNone3FGL J2028.7+1012?îÝ{EßKN?ªìÝ­wEÞ?¢(K¢K,?ªìÝ­wEÞ?ïk0nª?¤Uý¢4ø?'œùò*¿?¤Uý¢4÷?èXÆeý9?³£©<z?Μækì?³£©<z?î¦æ†û¹?˜mJ†›~a?¥'žgDr?˜mJ†›~a4FGL J2029.5-4237?ïÞšo¸ÀA¾#ˆÀ:͗ZBÀ=Ð&¡@Ö	³2@®ü*ˆj?ɼÿdύq?ïÿça"¯­@ìYÙ?üŒUc_?ïâTžgߍ?ÏkY?aj¿á矶êy¿ïý6AZ"I¿éނ¬Ã¿íœݰʹUNASNone3FGL J2029.5-4232?̗œh#]\?У0}Šó?èÚå÷(¨?У0}Šó?›Ž•)[q¯?°C¯¶j?ï#‹Vµ$s?°C¯¶i?ÏÑâJÝ?³ÖÂOCx?è:‹‡m}É?³ÖÂOCw?Tåm«?GÍ&
ëÄU?ïõôI*q?GÍ&
ëÄU4FGL J2030.3-5038¿î?N\Á·ÀB% …²À;MäSÒÀ<¾ßê¶ÂŸ@!üщÊï}?ú¶_¢ýÆj?È¢{1úy?«s¤i¡?ãè‹9"†@ñðÅûLg¿ïøª*s?ïý`t#"¿Ê;-½þR׿³½Øþ‰]a¿×(¹|ãÖT¿ÝáÉÿ={UNASNone?ïÿŠNs?˜ªT©ý±?
z},c‹Ö?˜ªT©ý?ïýûæÀ¹?Q$"9ð©?0 Éú7¹+?Q$"9ð«?ïòÑɲà?aYb7?Z\lš@¦?aYb;?ïùDR×m?@$™÷ßêO?Jî·ü¢M}?@$™÷ßêL4FGL J2030.5+2235¿Ð:üÆËÀ#yí9SÞ¤À;8
‡=À<'JŸ`ƒ@!‡'Kœ‹'?ð7`Sý®?àXBaNz?îLYµ@˜Ôw¼@.¶YBç[?ên^ýçKÿ¿ïñÊþ@9?ïþ
a'l)?pu¨ßÄ¿á'ïXèϿⓢt3®ƒUNASNone?ïÁ¼³>?zË8Q³?!·¦7àÝ?zË8Q´?ïë—IïèÙ?‹n|ÕG?dh¶'?‹n|ÕF?ï^%áæ!?v'TüZ?";CÃ=?v'TüZ?ï4¹-oÃ?'LõÁ8Hr?™hÚR¬?'LõÁ8Hs4FGL J2032.9-0005?ÞÈ"ÄÀ6tÅÉ£MÀ;nãª2À<f©¢%YV@ºãÓNœ@{GA1M?Ĉ\ÛMC¿£¦8ŽfàŠ?ã\g	#•?øÃÆ0{s?ïû<aZ8¿è»¸¨Rš¿ç!Ë+âÜÚ¿àÏπÜ3r¿å¦v î?¸¦g¢0UNASNone?ïüv®q?8íag'??$JŒwl±?8íag?ï¾'´Q¼?"^Ì27Žà?€vþ+Ñ?"^Ì27Žà?ïçðÔêtN?oÁÎG]x?h+‹²&?oÁÎG]j?ïx=#|-R?z¿²$+«¡?ø[zU¤?z¿²$+«£4FGL J2035.3+0557?èŠÚö×6À3ãêòQÂÀ:Ê°'Úb¸À<#à{Ö:@T­›"*r@͏ãÖÕ?ÄT±2<".¿ªÐû«©?äíò¼@®)Zvå¿ß²køvžÃ¿æ°ÕÀ'U'¿ïÿþˆ0»Š?ïÿÃÏÎ	
¿âgÿyÈC¿ðUNASNone?ïÿ¥-ÙÚ? _§÷ßÅ&?‹ZDļ? _§÷ßÅ
?ïýɋ§¼ÿ?R!Å-k¿?1³¢ÂD?R!Å-k¶?ïÕ(¨'*/?w'9Ó7ýÁ?uk«¾êèÂ?w'9Ó7ýÆ?ïÿr¿§`?"wÕý~tŠ?±¨ðT?"wÕý~tÁ4FGL J2035.3+0354?Ù\égl¯—À4÷Äâó¿À:éʄ0'À<Ii¦ŒÇ@âÝ¿
qƒ@(ˆÝ‰³s?Ç˂õ¾2«?™3èòŒ$?Ó5`F²?ýwVô-ŽÙ?ïúÏtFùº¿èΞÃO ¿ç§PÑÑ¿æI´´¨Ù¿ïÿæՌŽï?ïÿ˜ÁØRUNASNone?ïúžGX¼?H6…¶ûy×?E†âŸù
‡?H6…¶ûyÏ?ï°Ãéâ|¾?˜+…£spº?ƒÏ‡`ÐL?˜+…£spº?ï"ãOTû?"ælÔÅn?ŠüÇ,*Á}?"ælÔÅn€?É6<D?y§Ö—üX!?‰
²pï)?y§Ö—üX!4FGL J2036.2-0207?í>L´äÀ8/KøüրÀ:¿­FÈBÀ<dLÒJ»@}Š?©r@ï !·"?Ðx $Î?Ù{Tà2@Z&–m@Ý­)ï<¹¿ï§Ù}µ7…?ïÿáÍì¿à©ß'1.¿çôïËÕV¿ïÿõž}.)?ïÿxÃÐ¥UNASNone?î¤Æ"_9?ªÕ•¡Í?¥³—ºb?ªÕ•¡Í?ì'Å
/!×?ÅÄïR'Õ¿?»iז†ñ??ÅÄïR'Õ¿?è+?à áØ?²'`4ýÝï?ÏS|x¡?²'`4ýÝï?èj(µñy?¹&.bäœ÷?ÎW]½(:?¹&.bäœ÷4FGL J2036.3+5642c?Ó«Æ2ûûY@#Lµ»8PÀ:T˜ÜÛ7ÊÀ;ã·½q7@‹«(7V®@JNz·VC?О¿#@ø?ՈE^XûÅ@osۙï*@,ªžP8?ïÿøãú¿ÝòÅÅF››¿è6ÝâžÆ¿é@€Þ·°Ü¿ïGY•?å@\FQóéUNASNone ?ìó'Lê?·¶v#?¸cwşX¬?·¶v#?å?;Öòp¼?Ð×æ›&Àå?ՁˆR‰?Ð×æ›&Àå?âøQ#F?¸Ìé1A.×?Ú]¹ÓÅw?¸Ìé1A.×?çC`3è! ?´CÇ=`?Ñy?˜/¼Â?´CÇ=`4FGL J2037.0-2826¿ïܽ%ðT@ÀA3»¾‡¬À9âÓì{¾½À<@xã@¬˜@ßÿÆÜH@âE¿ý±q?»«É᤹ø?½ÌR֑?þ˜ªX-¾@%ô†O:¿ÙlÿiK¿äsãýjúJ¿æay,;È-¿ëeØÂ#{…¿ãÈ:@¿ïÿCÂw‰NUNASNone3FGL J2036.8-2830?ïþ›	¬Õ?'É`¤?&Oe2®ˆm?'É`Ã?ïý	;'GË?Sz6Ú,\K?7¶#mÁ§ ?Sz6Ú,\I?ïÙЇŠ5?qæ;—t¥Ô?sw—¼:å;?qæ;—t¥Ñ?ï돠ÙLô?UußÊ9Â?dp_&³
R?UußÊ9Ê4FGL J2038.4+4212?yK?á^wïû¥þÀ7çÇҒ¬À:6ÃákÀ@–¾Xéò@9Ó{<·@?·ÿvä܎?Ø+L'Œ@ ¤zž+Ð@‰ý¡O?èJ*Æ}'s¿Þ/–Æ€'q¿èHüލi‹¿éº\‡ÀSB¿îSfQÒ[¿É½‹¦¼Â¿UNASNone3FGL J2038.4+4212?ߣ‰´RmÉ?ڕã,!…:?à.;%ÖÉ?ڕã,!…:?"Ï–ŒŽŒà?¢.ž$Ñ°?ï¬Á¥ÍÅÍ?¢.ž$ѱ?ÉÌ;󣼧?³×	·

:?éŒñÖ?³×	·

:?#æaߚ?²E¼nº?ïþÏÓřâ?²E¼nº4FGL J2040.1-3137?ësW9z[KÀAèAÝ!êÀ:¹Åԋ0À<<š	+!í@ÐõšKpA@š(»
,ª?Í徶3®-?Á·-[?îÄùdŒW@>½õŠ±?ïq¢"¤À¿ç]tàQ¹Ü¿æ 0÷ïF¿éÌòŒyöf¿Þ†õw/¿ïÿ°_ïÉUNASNone?ïú¨YOÓé?K-òÀl1ë?E^šÀ°Z†?K-òÀl1è?ïÈH¶^é?'ï(æ:û?{ۤЋ–?'ï(æ:ú?ï8QÁÏ?'Q"§Ø .?˜õÇÜæ+?'Q"§Ø ,?ï¶ð?ròÈ#…àu?'Cù?ÿ€?ròÈ#…àu4FGL J2040.4+0312?Ülº	
:ôÀ6jǸÕ¦À:¶Ø¦ãÀ<5Cu –
@ FKé¸k@A3æÉÎ?Õjpr[g?ÑëNB-L?þ×]I‡2@St^v­Ü?ài
à"S.?ïšÅ³Ó׃¿ãúz_l¢¿áÎjüÎX¿ïû¼~Ëâí¿ïò&ޑoUNASNone?î'îÐ[É?­ù%¼¼ø¼?­úN"m?­ù%¼¼ø¼?înQÑOE§?·GZµÕ–þ?©âë¥'?·GZµÕ–ÿ?ëªLF?¨;#€ŠÑ?ÁWÒÎ忑?¨;#€ŠÑ ?é‡Á¹f͑?°õ™¹%b¡?Éàùdɹ?°õ™¹%b¡4FGL J2041.1-6138¿žÊ{6f£ÀBJ»˜Çâ'À:²Ìœ%eÀ<žÙç@/å(
eC@_ÀY÷Ã?Âz¦r	?±¿ÃúÁ'?ñ
£ÇðÄú?÷6¡þ»Ý?ïõ®£¿ÕoX½ÜD¿ã$À™+¶¿äïþ®Ç¿æ¸ž¬þÑ,¿ÐÀ£ÿN)YUNASNone?ïñ"[¸?Ws†b܈ÿ?\×ÕIƎ?Ws†b܈ø?ïaÎï©5ú?¡‡]ã5€?"Æ"
Ù@¶?¡‡]ã5€?ï¸ÛÚWô¾?±yn\c?É	jÐ7?±yn\cŒ?í–ð·uîx?•ûý"Õg?³HzDPŒ;?•ûý"Õg4FGL J2041.1+4736¿Ò¼¬AkÀé@¡QÙçgƒÀ8rZ¼8¨À;1hWØ.@˙>ªà"@ÊåN?°hÀ]ӚÇ?Ó*Y— @ /ˆTÍ·®?ûË°å"?ä¡þíÜ<¿Ñh–¾•¿á0³[â~æ¿æ*ü-¨…¿ë'€!£hпîmm¡n$KUNASNone3FGL J2041.1+4736?@hšœûã?3\æEÝ/Ù?ïûåÙ[ØÂ?3\æEÝ/Ù?~2
	V?š¯jÅÊ¿?ïÛåýíT?š¯jÅÊ¿?ƒZæÃm?géi3¸4³?ﲔeû€ó?géi3¸4«?A€'¬´§R?/Ÿûx™]$?ïûŸÛTÒ×?/Ÿûx™]$4FGL J2042.1-5320?éwm UA1ÀBãŸÂ¨†œÀ;RÂ}¾qÀÀ<·ä¼­šØ@ 3Æ 
aƒ@T@C¼î2?Ëd¢ÁáaY?"píÓ؄¼?Êg|;ôº?ýW
Éĕ?ï[}¾Ú¿æh/ßkµÜ¿ääo ÷±Ó¿â¢)?êPÁ¿ÅÚ»!ÿ"/¿çNV"uUNASNone?ïý¾zyk˜?1Ll¢îá(?2,4£K‹?1Ll¢îá"?ïùzE5à?h!GÅjýC?Jë(Ð$?h!GÅjýF?ïî_~~%?h÷ºbÓ?a ÚêÈ?h÷ºbÓ?ïì%@²›?Sñò"ìíY?c€Ú¿Me¨?Sñò"ìíQ4FGL J2042.7+1519¿ë—?À0F[¦ïÃrÀ:ÈLÃ'1À<a¸Š©@q®óñî@꟣žÖ?ÅÒVúb²'?±ÒH·©Ïó?î¿>¿Xp?ý%"GÍÊ¿ìà‡)T ¿Õ¼­šØ]û¿à}Tß«KÉ¿å@x`cíæ¿É߄_u±]¿é\_UÑUNASNone?ïô}ïr€3?R?š¿wž?W!ÿ˜Ð?R?š¿w˜?ïø_¾Œ'd?n)G‡) ¬?NÍöm²?n)G‡) ª?ï¼ø1f1?ñèe&?€Áó¦s¾P?ñèe'?ïÁ]¶°E'?p/ #«?Q$§Ý7u?p/ #«4FGL J2043.3-1520?ìëð.úhçÀ?sBí»ZÀ;"2.PucÀ<wìÔªà@ 2¯Øu@¼Iº^5??×£e_Ö)m?¹ÂH9€?åó s'õ?þLjKù'Ê?ïÃ[Ÿc6¿æ
d(ô¿åt%kÊSv¿Ü W xF¿èEÿ©þl¿ïþ^à`'ˆUNASNone?ïüYñÕ¦¦??	~3ŽŒ?=0qRÊËA??	~3Ž?ïÏÒ½@ž?'1²Ä¯à'?x¡_À1O?'1²Ä¯à&?ï¬ÖŽ™©Ý?"k'•6><?"Ê\Y•ˆ–?"k'•6>8?® ÿô?t$ž{ÍPÒ?‰UÔWÀ.?t$ž{ÍPÒ4FGL J2043.9+2051¿ã¤zÄzýÀ*ŽZݜ'éÀ;;øÒåÂÀ<«qøjàI@†å'Á@%Î_ª?єDuû°?ÝÝá<ps°@
e:í;Ø?üãô0¾å¿íÜiøÂ?ïÿ¨Â+‰¿Ú¢Ô`"ë4¿é\'!֝¿ïÿ×ñÃý?ÒDàPãUNASNone?íÁ0ß"¡?±¤ÈÛvvB?±öyê÷?±¤ÈÛvvB?åþðJ9Ð5?Ñ|Là֖5?ÔkŒ_–?Ñ|Là֖5?ã_ýÔµv	?»™+»·Ü3?Ù@V•î?»™+»·Ü3?ßñ˜IlR¹?¸iõ_΂V?à3ÛIÖ£?¸iõ_΂V4FGL J2043.9-4802?ï)Ÿwhš´ÀC$O"}ŠÀ:a'W«¸€À<Á#і`)@݀$¨€è?ûChjL¤ô?ÃOÜ÷'HB?ã"BwsÔä@ob?ùó:¥|¿ï±Óým©|?ïø®6Ý¿ÅUP~ó{¿äd­³,¿ïÿÆTǏ¿î‹EC/ÑUNASNone3FGL J2043.8-4801?¨G4|v?µÍ`áŒ]\?î{Ì¸8Ÿ?µÍ`áŒ]\?Ÿ…óù*ò?µ%Æ*•?ïÐgÈ6¨?µ%Æ*•?ª X¿-Z?›%nKŸ?îUút
+?›%nK?‡£Ù¤¼?|1TŒŽ?ï£ùqø™m?|1TŒ4FGL J2045.0+4202?ìÄìù'í¿à£öíóŽÀ9s?VW$ªÀ:ujhS@ Þ8¯õ@ªõ&ˆ*?»ŠgbèÑ¿´y€žP¸?÷쩬6TP@ÂúÅX8?×îyZ^ñ'?Ñy þ'bÅ¿ìv_"$m¿çZ"ö¥
k¿Ø*Hiü¿Þâ^D)UNASNone?é-rfÿdv?Ë0ðv¢p¥?ËJ6dn(?Ë0ðv¢p¥?î"ùêÓÄÏ?Áœ1·¨?§°aRó?Áœ1·¨?é>ÝAWv?¸FÉ?²?ËŠú¢'¦?¸FÉ?²?ïaï–o3†?†‰Á­LRé?"Â
2T?†‰Á­LRé4FGL J2045.6+2455?ìŠgY¥À&Sü–þµÀ:í§þàEÀ<L2Æü©3@0mUÃÖÚ@¬¤¾Éç?ƽRÜEæ"?úhDµw?ËVâðz§@¢‰,d¿êµ×ÙôÓ?ïÿH 荿臦†è½¿å"‡…¿Öû!sîf¿ïÿ⾦™\UNASNone?ïýRLÔ.?8[P—"f?5m™^
?8[P—"f&?ïý‹_E'Ÿ?Z£ x¥j?3¥Ókl?Z£ x¥e?ï½1J³Qj?C$ƒ9Z	?€³­S+¥g?C$ƒ9Z
?ïñ¼Æ¼R?Pfݓ¼V?\†sȇZð?Pfݓ¼V4FGL J2046.1-1626?ÍE\ÉÒû1À@Mz$‰LDÀ:n"B€À<~3Ѿ¤@<]ˆ¿?ÿÉ>¢Òþ?ÉÐ1[‰"?Ú`?»ËÈ@ÛÂ3×@®Â+ß?é:?A‰¿Ýc5ÄÝë¿Ó>âéĪ¿ålb©Ã]¿î65{âÏn¿ïüTyÔØ4UNASNone?æçØäl?Æè2#çN‡?ÒÞ0Oî7(?Æè2#çN‡?ìMÛ/Zã{?ÈRDÄ䗐?½'&…(ä-?ÈRDÄ䗐?קõ$!A)?½+ɉ³	?ä,mï_l?½+ɉ³	?ëþ°òD±d?¢çówÊv:?À<6í:p?¢çówÊv:4FGL J2046.9-5409¿Ê¹?ZضÕÀC3֝0'À;+m,SE!À<²ãô0¾å@ ìôèâÄ?úÏ÷>^‡?Ô'Jœ±Q?ΨZè	?þvÜG©ã@~õ&`è¿ïUtÁrüw?ïώH,¿|¿ãto=¥}¿ÒæV
ΐ¿Öz±!µR¿ïB¡YºUNASNone?ïö½eXN?PƒQÉ*ñ?S؅5Oc?PƒQÉ*ñ?ïø×1?ln›—Zß?OÐ£;ç9?ln›—Zã?ï°{Κâ'?€LÇv-¬?ƒáYG[i?€LÇv-¬?ï©irυI?v}ŠqpBÚ?…¥£L­¼?v}ŠqpBÝ4FGL J2047.5+4356¿ã9pµðŸ?Ô7.À\ÑèÀ8ÿ,íiZÀ:Tù]N°@"§âÅÂ@½Þ½ç?ÓÁÚ`3F~?èæÙóü¼@þÓr&Ž@²aôçž	?î_u`Õ,î¿Ôjãêv¿íÛX¡ì¿ç"¸+U`¿ïÿõÿ 1#¿ãL?bUNASNone?ÚÅ_@û?Ó\ñg?âP_'|ö?Ó\ñg?Ñ"îㄋâ?Ӆ
º°j?çnˆŽ=º?Ӆ
º°j?Ù§'œBՓ?´CêLõN?ã,>±Þ•6?´CêLõN?–S¯"ôӂ?…¸Pÿ"?ïMbƒXYd?…¸Pÿ"4FGL J2050.0+4114c?í;Ó¿ûá>ß8àÀ9VN>QtgÀ:÷b§K3@ˆèœa@s¾Ãõ¶?È?m©%Ó¤?ÍHMv«X@Ǡʃ?ý+Vøà&?áó!R¶¿æK>AÚ
¿ã-ðžc,ö¿æIWÍFoP¿êUÒÀá|¿ívYùp™ÆUNASNone(?Ñ}wºïM!?ÆjB~ö-v?çAD"ˆYp?ÆjB~ö-v?çyUó"¹j?Ñr	Aá2+?Ñ
T؍,?Ñr	Aá2+?àFÿ¡¹Û{?¸']¼ß?ßr¼ŒI	?¸']¼ß?Ò­õM@é?±u¯cpôº?æ©8Y_‹?±u¯cpôº4FGL J2050.4-3015¿Ã©yŽáûÀBÖxl"h
À;þُRïÀ<€‰Ù25Ý@¼N¡MÃ@³˜Ôw¼?Ñ{nOê?Öbºà;>š@¤³ÃçJý?ý²þ½wÅ¿ïÒ·ÈXÉÆ?ïÿLa¢—¿à'ÆN-Š}¿éѼ ¯¸j¿ïþªà"Ô?ïõfI
5
UNASNone?ïÀ§o|^?Î6e-ÒÝ?¬H{ÁÐû?Î6e-ÒÜ?î"È\k?¶;PøiAP?¦¿z9N!?¶;PøiAQ?ëÆ֏56}?§©´ð®[E?Àä¥Ã+&?§©´ð®[D?ë€|XRƒ?°Âo¦ù±'?Áþžµô?°Âo¦ù±'4FGL J2052.1+5539?ç|€Îò›$@móùa€À:¹‹U38<À;ô×°´h@ös%@vÅ#‹ƒ?Ðt4…Bʀ?³DS§?éŽmìl¥?ü/_"K|?ïìFD‡ïM¿â¡DˆÆ¿¿êŸç[ÄKõ¿ÔÄ5N–f¿ÞÍg'ߐõ¿íäñ@õh¢UNASNone?ïô)…ŽÙ?[€ÎcFÇ9?W¬õÆâNÛ?[€ÎcFÇ@?îÿòÈc?¶Ìâ¯JÐÌ? °Óyΐ?¶Ìâ¯JÐÌ?ïbÜS:·Ø?–Le>T?"¤u˜©ú?–Le>S?ïÕZ	&ã?ˆl3[µ?ŸåT¾Û#‹?ˆl3[µ4FGL J2052.2+1635?†$À1dô!-wÀ;
Á$"À<'=¢"@rò»ÉÅ@UÛpÔ~?ÖÊð¿\£?ïAÊsbÎ@Œ¿ôw5Â@†  ´k¿Èž&܍µ
¿å²¢\·¿áŸ¸Í;‡–¿ïÿyB=K?íöÛ>)±T¿ïþùoÃzUNASNone?î½°êPJ²?°˜Ø—kM?¤$ñZûTÙ?°˜Ø—kL?íe"-Eªþ?Ç&ÒèoÓ?´Öî•Ò¨?Ç&ÒèoÓ?âo¤îýR?¶"kV>H2?Û ¶"[Ô?¶"kV>H2?îIi§÷"á?¬`³Gp±?«ie€Ñò?¬`³Gp±4FGL J2052.3+4437¿ï'Ø'H?¶öԈ-
¥À9̌5-À:¯
•øÛ@Ì7Ž·"@"rä#*§?ÅÃdCK"8?Ý»ÐZöƛ@µQþÐU@<""†âÞ¿×°Ôßøà¿×¿!='\¹¿ç*7Á¸F®¿íÂÝ_¿ïÿºà¼ô¿í¦.}kæƒUNASNone?«y§Á?²Ï¢¸?îHo¯õƒð?²Ï¢¸?·.â^'E?śE×ç?í#´/·M?śE×ç?¼Ž	†~ö®?ªò°ãÁP?ìn>Ï0!+?ªò°ãÁP?•"(–}e‰?€ŸŒÄ8…?ïVî»LÔ?€ŸŒÄ8…4FGL J2052.8+5739?ä~¤‹$G@  ¦°)(À:ÉÈ5ŽWÀ;Á¡ùºk¡@	ý½/ ×@-°ê7?Ä驼ÒXÓ?½½Šåv¼Ë?úB¾ÁqNø@V¦í•?èç$œ—zÛ¿ã¥jÞR¿é·à†=¿Üœ›PÓØ¿ëùoÃzn¿ïÿÚ €UNASNone?ìð¯5å±d?¸Iïø£ø¹?¸z†PÒtÜ?¸Iïø£ø¹?ê4)wþÍ7?ÉÒU‰¤yE?Ç/Z Ë$?ÉÒU‰¤yF?ëÀ‹l¤n²?°&Î?ÀýÒMnE5?°&Î?ê´ü"Y?¦@ºvMû:?Å,v›¿ƒ?¦@ºvMû:4FGL J2054.1-4054?äJ_!"IÀCö FÇd®À:A…ô¡'À<_Öq'<Ô@´6"¦É@"*ú?¾!-¢$­‰?©s€Û¡k?낎»F"@n_.8Í?ïW¡!MW¢¿å'"¢‰­=¿çÞDÄU/¿áwáî-¿ïær$àŠ¿ïÚ8?ânUNASNone3FGL J2053.4-4052?ﱍM‡râ?ƒ2q…'›?ƒœ¬ž#G`?ƒ2q…'œ?ï¥g·"Ø?—ÜÄ
Ž?†¦Éþf?—ÜÄ
Ž?ï[ETŽ^?Lçp»Ä?"—Un49?Lçp»Ä?îÿ+KV?ŒÖJŽ)K? 
KJŸG*?ŒÖJŽ)K4FGL J2054.2+6904¿è}æWð'@.'ÄupÅÀ:Lµ›Wß»À<Eþ7¨ã¹@&˜®²@ç~äâmH?ÂF­¹a5$?Øó;Ì@ O‹XŽ?þo'€EŠ¤?è(wŽ'ÿ¿Ä®QM¥¿Ý·A 3fµ¿é'Û¿®×¿é"'?h¿ïÿƒ9UNASNone3FGL J2054.3+6907?‹NÏûv53?Œ<žœÖ‰7?ï'ÄÀ'+?Œ<žœÖ‰7?±ÝdÌ)ö?»èKbva?íÄSfzÁ=?»èKbv_?¹Ü@µy?§T±§K?ìßmäwéQ?§T±§J?qw?¢n&€ƒë\?ë\£¢>y¾?¢n&€ƒë\4FGL J2055.0-5218?í/MÐBœÀCèA¢a¿8À;>$'ýuÀ<‹î:ތ@¸ðá©þ—@ø&"»?Õވ¡y·Ò?Ñwûd9æ?ú«~3Æ@؋`pÙ¿é'Æýó¿½8¹›¿åãEf­¿âÚ
ݹ.4¿ïþÚ0bž[?ÏJùãÜ2ñUNASNone?ïýÐf5¦3?4Ý÷¿?1|ÎRÎia?4Ý÷¿/?ïý0¨,T¾?P­ö*Óo?6z¾Z²?P­ö*Óh?ï=éòÍi?Ž
F½Ò?˜_BÁ¦RÃ?Ž
F½Ò?ï÷Áè"?Cûo€µ—?P|.áÊ÷e?Cûo€µ˜4FGL J2056.4+3142?ï«'!IûÀ!£;u!MÀ9<›õšKÀ;»¹&&Û6@웺Iì@]!ê5"?µðR

ú?ÚÊd<Àz¯@ ì'éSQ@gŸÜ~ƅ¿Ô>$ކ³Ž?…¤éó'ù¿ä-–¦ Z¿è±càO5¿ïþ®û*®¿×']<9UNASNone?ŽXš›Ž?¦Àq¡•Û?•"™Ç?¦Àq¡•Ú?‡RPÒÄò?'ç€LÉ,?¼·¸ì?'ç€LÉ,?¨Þpåa"f?›—¡›é'Ö?îrñ©æÊ?›—¡›é'Ù?`1Ö)_Á¤?OÑM,Ã{?ïïÎ)Ö =?OÑM,Ã|4FGL J2056.4-5922¿æBiö*ÀCp¾´ .À:]¹À€Ž0À<yµIc @˜üsÙk—@Ý_á'?Å6ò…n"?ÉOJUŽ§Î@¢¢&0@u@ãJÇ?ïòÏàþ]¿äøŽ¼ÆÅL¿ã"xKtÈ¿áÄ x°ëÆ¿ïÿíöé	¿ælQaòc_UNASNone3FGL J2056.3-5925?ï3Á¾M?Ÿš»ã?™‡È?\!?Ÿš»ã?フøò×?–"
ÙM¨?€\ÁûƒJ?–"
ÙM¨?ìüÿ©Âú?¦-¦"æXt?¸±è,?¦-¦"æXu?î°%蚁?ŒèfÔ5²?¤ý¡vWî?ŒèfÔ5³4FGL J2058.0+3338¿ÒaÖÙ«;ÀU´$_ZÙÀ;-¶Œ§—À<¥"²È@ƒŠ'3õ@-@«?ÏíŒàΌk?یÒÁƒmˆ@	.<b'?ÿüW¯>q€¿ïÿà iA?ï¡ 8Bg?îN™á=@¿âåÃ=×Ñä¿ê³"¢Ú¿ïæ^£úE¬UNASNone?êïž!žà‹?ºÛ¤X়?ÄA‡y"}Ó?ºÛ¤X়?é'Â[-X?ÑÊú©^Ó?Éôö"ÇJ ?ÑÊú©^Ó?æ¸÷Ҋ‰?´pïükN:?ҏÎZêì?´pïükN;?àˆ©~8Z?¾±˜?ÞzK?¾±˜4FGL J2058.5-1833¿èRT—ò'ÑÀB¨ÁTɆÀ;÷sI£¸À<Ý1=­ˆ@%% _Š?ôÝWšÉ?ÑÇ"¾Æϳ?°U2a|Ú?ÑwÂd$ö@j&Õ+ëì¿ïÿõMõVY?ïÿ2æY¶¿ïþÛ½«q³?ï÷݇/3Ê¿Ýí¤2϶?¥'mœÕRUNASNone?ïÿ"	ì?T-p³ë?ý¿"ùÉm?T-p³ëÅ?ïüøקåZ?]ιÞÖù=?89BÀÕ6Õ?]ιÞÖùA?ïዕyo?mfV¬5â"?ntj†æò?mfV¬5â?ïü!äkZF?AÜH|U[?>ðÜ¥-Ïé?AÜH|U[#4FGL J2100.0+1445?ì=-;ÍêŸÀ3üæâ!ȨÀ:ŒÙ™cé´À<@HÊt,ù@ç®Tçî@…¢Ëqƒ?҄‡ƒí_ê?ß5ÿ–Mµ@È§¤X?÷̧¨.]¿ ÊŠÛÄ?¿àåê«%)¿æ÷çÝõ>0¿í'E.Þ:¿àèú}	@?Ì$ZR[ígUNASNone?í×7"cZ?µÃ™Ð@"$?±FC\ã5?µÃ™Ð@"$?èô2nbö?ÒLÑg¾ô?Ì/6FwÌ)?ÒLÑg¾ô?æ¿7-ž1?¶wwb^M?ҁ'¥Üß?¶wwb^N?Üðvx{u?À¨Ä,ÿ?áýÄÃÂF?À¨Ä,ÿ4FGL J2100.0-4356?֗­˜Ö­0ÀDŽDR?gõÀ:{®•ª ÐÀ<s"vD)û@¢©"P¯@Ì"û­Šè?Âă½B(?±äÖ?íÛ{@¾>?öÈ¡›@
¿å²À?à¿åN.â´G¿åCì>Bu¿â.'Z·Ü{¿ëŽ'Èê¿ý¿ïÿV"tnUNASNone?ïÒÃÜ>Û?rfœˆ% ?vžðà';?rfœˆ%!?ïd º)ú?¤ó¹þ~•?"{èºÌ@´?¤ó¹þ~•?ïf¡rƒ8$?ŒÐÓ9ycÌ?"+ѯ˜û…?ŒÐÓ9ycÌ?î?tr<`?—$ß»¡¸+?¬ø¸Ü9ø?—$ß»¡¸+4FGL J2101.8+5044c¿í–ï$Z|@½šzj)jÀ9ˆÁe}'À:Ø´«m×t@˜^IŒ¦@"¼¡Ÿ?Ñjþ;.Õ+?ҁõuü@5" ¼8@€ˆ'tð?ï¿ø="ßE¿ÕÔ~œéf¿ç|΀2À¿ë8–IƒÑ¿ïúmN·óø¿î2í"ñÚUNASNone(?㘻WS|¾?̜Î4Oâ?ØΉQY'?̜Î4Oâ?×GÐ
Ih?Ñy†´	N{?ä@\úÛL?Ñy†´	N{?ÛdñLƟö?º5*"®ß™?âM‡Yœ°?º5*"®ß™?Ø	ÜÃB:7?¶n'±¬éá?ãûž^âå?¶n'±¬éá4FGL J2104.0+4623?îpžÑ_8¿Ôj"m¸j?À:<»+º˜îÀ;¸–ªÑÐB@Îäõãq@:µå)»?ÏUöV³ëÕ?âVr¬MÑ@ó-¤}ù*?ûrA>¿åÜÁ6–•¿âiOBÇ%¿ÞKZÓ¿ènq'yAŠ¿ïÿÿ" 5•?ïðÔ^;Ÿ"UNASNone?ß©-UP€?Ñ$R/?T?à+iUWžÀ?Ñ$R/?T?â…Pʳ>¼?×fýð9å?Úõ^j™'‡?×fýð9å?Ó.Âç?¸ÕUóúÒ?æwhžŒvø?¸ÕUóúÒ?ن祼Ë?À"½}â?ã<õŒ-!œ?À"½}â4FGL J2104.4+2116?é%íÚåÙÀ0ъeI/õÀ:cÖ1riÀ<3­¬v0@ &J4'æ@çÝÿú÷ƒ?¹¸‡E"©¿ Ëq>AëC?èÑÌ`–BÍ?û‡«¸°¿ïç:ÁòÔ?ïþ|ý׆º¿èktøÐ`Ö¿Þ±ù⯍!¿ß­j0öB¿Ø0~ã"õUNASNone3FGL J2104.7+2113?ïòu'S¨?U/¶;qJ?[ÖÛX¯r?U/¶;qJ?ïÁÏßhÓB?˜[j5-ò?K–_?˜[j5-ò?ïÔÈÔ²½I?w}=ŠWݜ?u›•¦¡[¾?w}=ŠWݗ?ï
[e3?íhÓ÷MW?ž´œóYœ?íhÓ÷MW4FGL J2105.9+7508¿ïþ>iÇÝÝ@2S^"ñÀ:+Õ£5#ÎÀ<8(¾e*ý@5¥›ÛhF@"}ÔA5?½#qõáõ?¨_¹<æÔû?î˜p9Mÿg@y®$û¿âßßÏp¿Þ)«|ñ¿æ~"4­†¶¿ÞàÙ>Ú[¿áíks¡R¿ëZsž³3ôUNASNone?ïࢷÒÇm?cÇE+_cÇ?o]H-8"=?cÇE+_cË?ïëâöm?€­Ò¦‹?d	ú'ø›?€­Ò¦‹?ï¹­w?Û–kX?"¢?¾\A?Û–kX?ï7ÛæÐK¼?ƒì–|uËÀ?™ƒ%öˆh?ƒì–|uËÁ4FGL J2107.5-1507¿ê'$H&ÀBn;ÑgfÀ:ø0ÁhëÀ<2¨J6"÷@ ø(›)½@՘ZÕ8¬?ÂaÓY®Çÿ¿»¹f®_Ï?ýî}÷|¤?û}/և`²?Ò¬æ}wúã¿ë¡É¿îZU¶ë¹ø?ÛlKU‡¿æOËàÏ»¿ÃàS<h5UNASNone?ïëÓâžÎ­?eî>Ò¯ÕÁ?d,a1R¯?eî>Ò¯ÕÅ?藍÷`+B?Ÿ3c…e?†×'õ/ã?Ÿ3c…e?îüˆ-2Ä?•¤©èæÁ? 7},Ó¾…?•¤©èæ¿?ï»Ä—S*×?}# ûæ?Ú+5J
?}# ûç4FGL J2107.7+3529¿½Ø£ï7µ€À A_ˆü"dÀ:~¶H&	À<
ÿÖ"î@P@".þñ@È"ä0–¡?ÈzyBáüà?¶ÖÖ»ãñ?ó"Gö8Öá@  BU:?êDã߸⵿ٍDv§|¿çM}ŒGÌ¿ì	áàÛ!¤¿âƒŽ_©³Ã¿ï«a]*UNASNone3FGL J2110.3+3540?ïóƒ'ƒ2?Yº¼´ÒQÇ?Xù°ù›×í?Yº¼´ÒQË?ïþ:õ.?J>›'â]€?',P¯?J>›'â]y?ïR¸|?ˆk²‰ÉC_?5¨ð?ˆk²‰ÉC^?ïù¨å›ù?7zÙ&?I\ió?7zÙ&4FGL J2108.0+5155¿Ýú÷–sÅ@N>ò"{À8í̙¡&VÀ:vF›ÅÃÄ@©PÑ~¸B@:ÙºñØö?À\‡ÀSAÆ?ÐßüÉï£@NÅ£ßâ@
¢›Jõ¿ïⶮ}Vm?t¼j¿âþÚÁW"Ò¿ècê?ú@ù¿ëòpK™¿ïõA?æIöUNASNone3FGL J2108.1+5202?†šÅ!Å?—ðv±‰Fä?凜ë{§í?—ðv±‰Fä?¢6³M,ü˜?°1dJq/Ü?îܔË-06?°1dJq/Ü?®±RS¡ÿ¶? ‡/§ú?îêÚÅà? ‡/§ù?»¼õãÙh?«¤á
§a?ìˆaC"Òþ?«¤á
§a4FGL J2109.5+5238c?ÉæÁÙxÉÙ@	ݜþ¨çëÀ9W"¥>ŠÀ:ÄXÉűP@]±°ç"ø@Ò¹ƒCì¿?ÆCß=g¿'?µžÃúì?ñݸ'#Zx@DgE‹%?îè¹AՍf¿å%nN'4¿å÷ìÀÞ(¿ç¸Û^
!l¿ìӄABÀo¿Ýޘ|84ÐUNASNone8?ëlk8—ž?¿<ßQTÔ?ÂNS½¡Š?¿<ßQTÔ?ìhi¦¿æ!?ǧòOi%›?¼¼²ÊÎþ?ǧòOi%™?êlxu?±i\«@g?ǛúN-?±i\«@g?ë­#†‰ï?§ZÙd¤Ï?ÁKqçØF?§ZÙd¤Ð4FGL J2109.6+3954¿ÒYÀgí¿TÀ¹_í¦a(À:lf»ö»´À<PÍwí@"`´á¼©?ö)`F'µ?ț	›µ'À?ÔÜo×ÿ0@f}þ2 f@hH0p`:¿ïÿ&DÉ^?ï÷
ø{§¿îÃ`!¨Ç4?éìu:'Ä¿×C­¿@r6¿ÛªŒ[¨¾UNASNone?ïinéû?'êl·$@?'Ò"ÝN@œ?'êl·$@?ï¤ÓªÏQ?°=éæٓ?†Ë=ÕL+¢?°=éæٓ?ì}°Ak!?¨-É"ùÐ?¼2}ô¦ÿ?¨-É"ùÑ?ï•/È>V2?"äüSm´¤?Š´
ðjsj?"äüSm´¥4FGL J2110.7+5129¿ß+,ÑOÅ@ƒڐڮÀ98CEÏíéÀ:aÉí{ì@À•ý­ÀB@¬ dŽõÒ?ÐÏòñúƒ¿?ÚiÐ1Ü@
ïB-¡ú?ÿdÃo?ïÔ.öw¿à†h>ح׿èö=áâß¿í֎ín-¿ï÷/væk?ï²Û‰þñãUNASNone?é¢ó›:ã?ÌLá|hh?Ét1"sç?ÌLá|hh?ÓÛ%ø!}?Õ#Ôà—0Ô?æ{íïB?Õ#Ôà—0Ó?×ôUÕB?¶z°xޘ5?äÕpÞÂ?¶z°xޘ5?©øtº??žœ?†šÂ?î`x¶ô_¬?žœ?†šÂ4FGL J2112.5-3043¿æ3U}r!qÀE8Ɔ"ÄÀ8¹}'âïÀ;ûK¯Ri@æDÖ ³?ù?<;±'?«é³@pž?݁b ß9@1== ò¾Ï@'wVM¿|¿Ý¸çì
?¿ç¨eÜÔ¿ÄTÌ '¿àã|aO{=¿í/à˜[¬¿ïÿý±q&´UNASNone3FGL J2112.5-3044?t|£b¼º?pì L©Ô?ï×¹;ֆ?pì L©Ô?jÅGܺÉ?…`zE5^¦?ïºTêà?…`zE5^¦?­fAHғ"?£a:cöî*?î)›ërÖÇ?£a:cöî*>ÀžyM:^>߯¢`hÖ?ïÿûØy!­>߯¢`hÖ4FGL J2114.3+5023¿éUÊvÊ?òaKßÒcÀ9n‡–aÖµÀ:é×5Ü@£Dîq6@±3™Š€!?ÆÖáM¸E?ЫÈÛ¦"d@×"ƒ¸†Å@¥¤ªCàÕ?ïvŸ~µè…¿Ý[òú³åË¿Þˏ(ýO¿ãÏ¿®2¿í¾‹Ái¿ïÿ ß‰
UNASNone?¸±Rv¿Æ?·^f›íÛö?ìéÕ±(=?·^f›íÛõ?ÚT=ï"Ë?Õj~‰,=,?âÕá~n›?Õj~‰,=,?ÔXó"3?¸ÌV[HÑ?åÓô=æ{?¸ÌV[HÑ?à–ßiUAL?³)¥j×?ÞÒA-U}f?³)¥j×4FGL J2114.9-3326?֖oP/ýgÀE¬§?tŠÀ:Xš`hödÀ<QuÍâv'@¶²}k:·@¦¦Bˆ?½~ßrۄ¿â±†J‡?ÆÜô7Iî6@»Ÿ/Z·?êJ7&úƿ֔øà|-¿æZ*M±c»¿Í"‰ê}7¿åà• ãû=¿áÆëvÛÿpUNASNone?ïõS®]O±?M,%O'?UX£E`œP?M,%O'?ïýy´¿Jü?NXMªÞŽ?42Z¨Ò?NXMªÞ‹?ïï×u#ÎÖ?k~™Òö}?`(ŠÜ1)ú?k~™Òöv?ïêEãÀú°?R_g¯X?eº?NÊ?R_g¯U4FGL J2116.2+3701?éüŒ<ç-À ®˜ÜÛ7ÊÀ:"܅§tNÀ<=èõ!­@&*yPMö@ê#×u?ÅÒîNý"?ìZ0Fï©@"­`ûH?ùk5X'¿áF´"×j¶¿Òr‡[ÿZ>¿â7WOr.¿ì73"l;'¿ïígwžZ¿ïÿïXzUNASNone?yä¾úý*#?­nTGÅO×?ïÌ6'
¬?­nTGÅO×?'uúđd?¡C+v×?ïlWp)Ûu?¡C+v×?"FX—Å?¯L&#Æú?ïÃ]Í;B?¯L&#Æô?AóJ`G¾?0@ù¶¹Ìç?ïûƒ-xgï?0@ù¶¹Ìç4FGL J2117.0+1344?Í€²H/^À7Þs×ÛõÀ:{Ì'‹_DÀ<Dô·ÍaG@²‹'Ä
6@=¢ø½ì_?Æ´©Ýßo?ÖÙ`®ìg@ìJ[mäà@ÃHïÝóç?íœK9¿áx¾'²!¿â<۝Ëœ¿ã¢–b­tB¿ì±–`)5ƒ¿ïÿÿ«FjUNASNone3FGL J2116.9+1343?áBò2ä´?ș·p§€?Ýz›ü6—?ș·p§€?ìQ0Y…Ó?Çk^@?½v}3Ñgå?Çk^@?à×óäGL?¾jºƒ4Ž\?ßôP7qh?¾jºƒ4Ž[?ìN¬zý9? ÏMÊu½?½Š›ô(3? ÏMÊu½4FGL J2117.1-5307?ͺф¼bÀE~\|ؙÀ:ˆL€À<'|»@ð–ºìû@	­þ«l*?Á¡ËiM÷?´®!7?õ­·þßn@o¥'(^?߬:›‡Z}¿Ñ¢[Õ¾¹¿æSþÕÞn¿ÑÆU#óпä¢n>÷âz¿ïÿ²gƸ·UNASNone?ïÿ(V;?§d_l«?¼úõ8‡‡?§d_l{?ïýõ!765?Khbʕ)?0VöFNP­?Khbʕ)?ïó¨âùV?e''
ڏ?Yخ:
SB?e''
ڝ?ïò3ÒÆ ?F®=9ûq?[™ÔZrÂC?F®=9ûl4FGL J2117.9+3729?×DÚví²\À ŒFŸ¸À9žY …F%À;Ù ™hr@}xåÄëW@8J"xÈi?±«HÓ=?¿Téf`‡)?ûMÄ(¹\®?ñî¹Ç—¹?ßèGœÌ©ç¿áJ™¶õÊó¿àÙ๨¿åÉ£ý˝M¿íǍþZäR¿Ã·¹Õ¤6×UNASNone3FGL J2117.6+3725?èâ.£ÿ¨?ÃA£‡÷Ò)?ÌwG¡p`?ÃA£‡÷Ò*?è"ҏÇÅ?Ò)°lçì|?Í°¶Ààî?Ò)°lçì|?ënG')ó??«2îŠ;ùè?ÂFãcX3?«2îŠ;ùè?زìí>ƒª?µèœ21¸?㦉‰`¾+?µèœ21¸4FGL J2118.3+4055¿ê\	¼»ÀÁ)/»¯À;-î@ºÛ3À<j¦'F•ç@"OÄÄÂZ?÷eâ}8:?Ӟ)`ÌsŒ?Ó|]ž–¯?þm‹ÕÓÝ@úÐ<BüT¿î‰
€6œ¿ïÿý¡UûŠ?ïÅ!ò6?ïÿ"ÕåzC¿Ú×ÄØ6¸¿å[ח+*PUNASNone?ïú'Tðo†?@«+DOÝ?Eº¬>AèD?@«+DOÕ?ïüú€"ª‰?WÒc4Û?8+ûÚ«¸¤?WÒc4Û?ﶌžúÕ¾?ƒF±X3Ù!?'\ØAJ??ƒF±X3Ù?ïôƒ°Z{Ï?Q÷´U4|?VøŸKa?Q÷´U4{4FGL J2120.0+5257?ïùÒgôÛR@[©ßaúÇÀ9?踻ÐÀ:àF3À÷¬@SN×(›U@äõ$ÚªÜ?ÆF—i¾?艀qÕZ@"·þ®û?ö?ÊÎDò?ï}{áwÔ£¿×ïÈdÞ&¿áÅòÞ.t¿êûÒï)¿æÄþ;â¿ïÿùµc#¼UNASNone?êñ4X1ø?Ã+Ûªpû?ǐ;.Ÿ8 ?Ã+Ûªpû?Þk
ù¦?Ö81Àq{h?àÊ9ys-?Ö81Àq{h?åa5'­ƒž?¸9²Ÿ=œÈ?Õ=•°¤øÃ?¸9²Ÿ=œÉ?ÆBFgÚD?«»­V™?êz¯nf	p?«»­V™4FGL J2120.5-0138?ïà"@"ÁÀ@¾&ÉÀ;9'ôcê‹À<ž3>íÂ@!ÞdNß?þh7‹‡ˆ?Çh1ôo¿‰Û—.ʹ?ÃfýNÉ@$`Ρä¿îâÅÝo\Y?îY¨¿ãVöâv¿ÞVé†@÷A¿ÓÜ:¾l⬿ÌQü)ÝUNASNone?ïþ›"ôO;?%y"
ÎS?&MлR"?%y"
Îh?ïýr"Õ´?SLõûÂê=?4kYW:d%?SLõûÂê;?ïð°|ú'o?cm¸i¨?^Ÿ
Ý"Ý?cm¸i§õ?ïôã\‡G¹?JJæaA›¨?V9Fñp?JJæaA›£4FGL J2121.8-3412¿Ý/ÝÀFp(€QÉ÷À;É%,à2ÛÀ=*"¬ÊÎÆ@ £~‰x?ü—£U>S?Ú¥‹-lË?ïþáQ¿u@#È\$Ä?ý=ÓLKˆ?ï=è΋î¿ïÿõƒ¥;Ž?ïþìɹ¿Ãbý±@¿é3çcQ¿ïî´³ÑSDUNASNone?옴#î54?»¹(Ùë;e?»:^àŽV`?»¹(Ùë;e?䮔¬ÒÃÝ?ÖtÙ©ú—?Ö¢Ö¦ZxF?ÖtÙ©ú—?é6ÆMðãš?³Å'©jâ(?Ë$æÈ<qœ?³Å'©jâ(?ÔXòFÿ–;?Ã"g|Á3?åӆ܀4ã?Ã"g|Á34FGL J2122.3+7653?Ýöb-iLV@2²IÂÁ±À:ù» Tž¾À<{:r•@0Fþl,#@£a~ ?Ëüð@šNö?Æô·7_?úk©f–7@ôÿý²¿ïÊ,¿%Å7?ïü% "Ÿ½¿ã[Š4¡È<¿ä®‹™%Ö¿ãÁöD•[F¿å™Ž´/óUNASNone?ï­ÐZÆ'?†‰_°
B?"‹þ©Nv??†‰_°
B?ïì9n'?"û5™åé?cúrƑ}¡?"û5™åé?ï h^´'?•ËõìF?{òô)m»?•ËõìE?ïUê0¼s?'dñ9Ù#G?•B½Yèq'?'dñ9Ù#H4FGL J2123.5-8315?Óñ¸™èöÀ?$-òˆHÀ:ÍF«µûÐÀ<7™èsò@@ûEاK‰@¼Þ…[ôó?¬DµÝr¿£îî¾AÍ3?á3W{V@¾'$Ý¿ïýýÇ@›Ò?ïºa¤µ¬¿çÅä Óõ‹¿ãÝ}‰˜š–¿àì1¡¸¡ó¿à·Ð]óÑUNASNone?ïñþ
þ(Z?_ýNl&Š•?\ê¯KÖ?_ýNl&Š–?ïý#ãžÈ?TwM¸¥Ù?6ç0ã	Í?TwM¸¥Õ?þÁ_y?NŒ{P?Þ@O¨!°?NŒ{Q?ïë†W¼³'?V¡¶uv'?dy¨CLné?V¡¶uv4FGL J2124.9-2433?ÙÚÿ1љÁÀEå.rÚ0À;sjZç­À<‰M DC&@‹/ûh@Eˆãhð"?ÒÞbKy¦?ž‡ô¼¼²?Å8L7;*£?ûB"°Ìf ?Ë<*'ÆÃs¿êÍø{§@K¿×úÉ?#¬X¿æYlÀd¿ïýñg¶È¿ïæÿ8mUNASNone?ï÷5ÝdS?T(‹²ã?Q"EÁ7[b?T(‹²æ?ﻁß'¢þ?•…Ô0˜>?ˆ6@m?•…Ô0˜=?ïLg(ûé?±Rš_9?–sàžË?±Rš_5?ïŠób h?xõÐ;N7G?C'wùæ
?xõÐ;N7E4FGL J2125.6+0458?×k'[]…À>Ü@¿ã°>À;Në¯æâùÀ<˜%·I­É@ ü´fú`?ü‹Ë*5]°?Ñý6aé?½¬ ›$´?îƒÝo²@?þH%Ûܵ"¿ïÿúVrÓ\?ïþ½_ÇeÛ¿Ïe
gs¿Â%›¨±:¿ã3ÁˆK¿ÙZã¦XUNASNone?ïÿPqjǵ?¦-EK3#?ñÒ§	M?¦-EK2ø?ïø³ËVšb?m&¹´9i?M0Ò¥–uY?m&¹´9h?ïîášS€[?dÁd"y?ae¬¥+?dÁd"v?ïÇ.Uò?jæ)2cí?|÷hÕ`?jæ)2cé4FGL J2129.1-0240?ì™o=DÙÀAðuöý!ÿÀ:«åüjIÀ<=²¢i@ƒÉeeà@ÝäÅ©?ÈTí˜oW?´˜|c'í…?æÞ|Ý¡0g@	j
fEj?ï°~¿å±ú´f¤¿èf££׿ïÿ¬óéqH?ïût_ÎFÊ¿ðUNASNone?ïÿÖ'ªZ>üd˹U>ôì*Ò·Ò1>üd˹?ïþ¯ýªÅÕ?CâžÅkð%?%%S¢³Á?CâžÅkð&?ïÒËŽø?{öžÈߪ¿?vš|8ƒ÷œ?{öžÈߪÂ?ïÿ§™o-²?´[XÀ-ž?¤4"ž"?´[XÀ.4FGL J2129.9+5833e?ÅûäIèͦ@U›¡±–À8¯Û$~eÀ:Òe횢®@ÒqdFPœ@)Ưc/?³Hª~CQä?·˜¤Òód@ÏPB7²õ?þk‰0?ãÆ¿"9C…³*¿ÝÐ&^
§]¿æµV¬µ¿æéìb"IÏ¿äÒìnºÉ?³õR'AUNASNone3FGL J2125.8+5832?êTW"*̾?Á
p@*?Æ®£wTÍ
?Á
p@*?à{%ðây1?Ô¢Ú|ڋ?ß	´;
ž?Ô¢Ú|ڋ?çd×&·2=?¹ó÷¦=?Ñ6Q²'›…?¹ó÷¦=?ä[fI6ґ?¶D<Ž€c?×I3m'ZÛ?¶D<Ž€c4FGL J2130.8+2649¿v±WÏÀ1¤÷‡‹zÀ:ƒcj2£ÁÀ<T^üå™@8²yŠ@5!¬ˆŠ?ÖëU£öiÔ?Üýi¸*~Y@¢0[è^#?údW†¤Ÿ?îpï ´«n?ى+¶c¿æ˜ZRp¿íßø="ßE¿ÑƳãÇ»¿ïÕå¯ò¡sUNASNone?æ\3$±"?Î¥/:Áb?ÓG™¶ºþ?Î¥/:Áb?éÂò``?͕$|ì®Ñ?ˌô6¶'?͕$|ì®Ñ?ãaŠ©ƒ?»YO íà¨?Ù<ê­Ìù×?»YO íà¨?â`i÷9¥v?À¶1"°?Û?,Œµ?À¶1"°4FGL J2131.4-1124¿ëîüú»7úÀDN#c²WÀ:½T#mÃRÀ<aUy¯‡@cD¢œL§@¬Š7&?ÔÃmãæo?Û(mÀÍ»@9?l&™È?ûëg\…'û¿è…–½q:*¿Á¢Ú›¦º¿åÕ<Kv¿ëÙB[Å"´¿ïÿùJYQ?ïÿÚ@RÖgUNASNone?ïY^û"B<?™3Rœ¢å?"Ô w¸}?™3Rœ¢å?îy;ó…j?·h@Í–?¨n<@Ç©L?·h@Í"?êîí˛Ñ?©âÀ–Ò;?ÄDJѐ¼?©âÀ–Ò;?ìp2'?«ü{°î·Á?¼Ökq?«ü{°î·Á4FGL J2131.6-3714?ïðÌÓ,q=ÀG…WÞ
fñÀ;}ÁÅìßÀ<±ËY/F?@!B4éì˜?ÿ "•MÚ~?ÇB$½¤Ä¿¥µË\??âyÆ?"ë_@É͓ò?âh®_ybB¿âoçïhH¿äþîÝî³'¿â¥w=¤%d¿ïáÜÿI÷›?ïÀ­TžéUNASNone?ïý¤¸‡jÉ?7m¥ÿ?2Ú;Ä©ºX?7m¥ÿ?ïó5ÎrÜÑ?sy>ÓÛJ?Y"cF_B?sy>ÓÛM?ï«õ«I°	?…"MÊOùŒ?…•-"ýÃ?…"MÊOù?ïìVB+ú?`<',Ö?cÿ©½ÔÁ?`<',Û4FGL J2133.1-6432¿ÛìØ°n#ÀD¤øßzN{À:Œv›gÐÀ<‡Tn^@tG]â‰?þ¡ú@£^>?ÀV9ˆý?äê^x[[p@r)AAé¯@0ì1A?ïü\ý†þâ¿Æ"œY½`ž¿ÕD«@5$O¿çŒ |aû¿ï"®"g³î¿ïÿÔÌuŽøUNASNone3FGL J2133.0-6433?mLQ×??r"O@¯¾¨?ïâù³r®)?r"O@¯¾¨?Eíð"Êî?¡(òO-k?ï}А{a¨?¡(òO-j?•^¤ôÊ1?‹6D†¦?ïU
ØY¯?‹6D†ª?xKƒd±ñ"?exh­#QÚ?ïÏhù6œ?exh­#QÚ4FGL J2138.9-0408?ë©¡FÆÀC\ó^1
¿À;VÏj5þÀÀ<¬àŸèh4@Š ¹ˆø7?úC(ùôMD?Ý3ۀnÐ?æÁqðdx@Kݞ¬(@]wõ#¿ïÑ
ŸYƒ¿ã•Ð-hï?ïïñʳ¿Ö@›Ñ'>3¿ïü–ä•¿ðUNASNone?ïþ@E7?3¬Í|vÑ?+ö+®zW?3¬Í|vñ?ïù"'ÿ±ç?mü"E™×?I­ô8dØ?mü"E™Ò?î²æ+ßMN?—œ­‰1. ?¤ÑB+)?—œ­‰1.!?ïœã·E/?ò‡¬+^?ˆÇ?R.´?ò‡¬+]4FGL J2141.4+0733?嘆˜³À@6*Ã") À:…ì燫À<4ÛE5"7@kTù‹±@:aàŨ?Ãóʨku?°‡D­Y?ä¬é¢Æi?ú|=•âªÛ?ïÿtõubƒ¿Ûh(]lAÈ¿çì;AõmÖ¿æL,ÿ<Œ¿ïÿõEq#?ïÿµøtñDUNASNone?ïúÅ­IrT?P¢éw´Cì?DéJÚ6¯0?P¢éw´Cã?ï)+Œ(hþ?§øïÁkm@?šÚŽzòàA?§øïÁkm??îÙû©xIo?•V¥)tÍ?¢`Eh{i?•V¥)tÍ?Ÿ`¡¾?˜ßþû¦Œt?§Ö	õä ?˜ßþû¦Œt4FGL J2142.5-2029?îNJ,\ªõÀGEŒÒ
ú/À;oA×:åÀ<ŸÒcÃ@ ´í6y¹ª?þñ#Xʜq?ÃN	M[¨¿'á´+ì?Ë2að
?ù\ò3Ž£¿ïÿÒþÀù?ïÿüÚ±'Þ¿áL	Þ¦%¿åÁ(ôëÏÇ¿Ëì쥿Ëiº¸M9UNASNone3FGL J2142.6-2029?ïþ´šå–?#\2-OS²?$¶^¡¦®¾?#\2-OS†?ïòPx)F?tBâqØÖ?Zá_­tî?tBâqØÖ?ï¿íÝÔ
A?€åò¾?€ˆŠü¯Ö?€åòº?ïÕhŸ|?iß[îm­œ?u~Ëþ0B
?iß[îm­›4FGL J2143.4+6608c?Ê·ÚÊyW{@#¿;ÉêpÀ:üíüÈ=À;¾X0ë@ÀU9@Þ~bÜn+?ÂÌv¦$—d?¹ŠÔø³?ödˆu"ç[@É2Vˆ?åguZ0G¿á~¸+¿ä߯þ_ìпêDùdŒW¿çE˜%%Sw¿ÅaŽ:jßóUNASNone ?ï™mïFÃ?†Zêbà€?‰¤».Od?†Zêbà€?îçvß?³­Ø~G"?¡èžßò?³­Ø~G"?î‰ï ZŸ?ž|ѵœ??§n
úV?ž|ѵœ??îŠl\Ð{H?9(«*Ç?§Y:2øK‰?9(«*Ç4FGL J2144.2+7709c?ïýX]§Ú|@2.bÀ;y⏬°ÎÀ=6.Ú²@ #apˆSK@7#û‡Ë;?Õs4?¢­??ïþÑa‡•@òS—VÉ:?÷՜NÕ¦¿ïÿÿ&¦³?ï芘tÖl?ïÿ§ B€-¿Ô:©´™Ð ¿ï€]óÑ"?Ý+%þAcøUNASNone ?ËeOùƒ?Ë:lj³Y?é&¬½Ûß?Ë:lj³Y?»Òˆe
Æ_?Ì|3HŠ‡M?셮ó^G4?Ì|3HŠ‡M?ئø^,¨?¹ÙCÇ?<1?㬃Ðöi¬?¹ÙCÇ?<0?–r-?ýsé?Œ)ƒûï¢?ïLn–`?Œ)ƒûï¢4FGL J2144.8-1600?ï&)lB0¥ÀF¾÷øËÀ;u¬QéØÀ<µ
qs	ã@ ¡¦a(9?ùú¡¡¥×•?ß;m>qÕ°?ÔrcÞ=?ø™&âÂØW?ûZ$¬1̬¿êï<-­¸5¿ë†®Š©<¿×¯•¤—y"¿ç°¹`´JË?ÍYjªmÒ@¿ïÿþR€ÖTUNASNone?ïûރ6›Ü?KIÖ?]æ?@…ó%ŽÒ?KIÖ?]ó?ïöÀbP}–?på'ç²é…?R;_Ô!?på'ç²éƒ?ï2tÇ?"¹6É?Ÿ]™±g÷?"¹6Ê?ïé­?L
®?cˆª»Ç?fRÀ³òR?cˆª»Ë4FGL J2146.8+4808?ï|¹(`ƒÀ}	@¢CÀ:oD"n¿ÑÀ;È[ז@FE}@¥1Àll:?Ç7ׇ»Ëž¿…ðYfE%Æ?ÁÊTâÛVþ@#J|ù{¿ØɁÿ-½¿Ü@ŸWs¯¿í±VNÁ¿¬Æ¡~Y;¿ì­×^v-?°žª`Í[yUNASNone?ï"0Ìú'É?Š@	_°š?ŠóÌÁ_N?Š@	_°š?ïù«'¶ª?p´ýst\?IQ·…%Vü?p´ýst\?í©=Ex·=?¢,o´þ?²¶Ô:F?¢,o´þ?ïéß|ò€?\9ŽL?fë ƒ
Ñ?\9ŽL
4FGL J2147.4-3854¿êPêö­÷ÀI\лnÖÀ;Ij­À<†,9
ä@!ÅX^è@ÈÈ@vÕ?Çãr€¦´¿Ÿåg}+"?ÕXTßd@IqŸŒ¨¿Þ¯¸¿ÏŽH¿ÞØs/Àã¿å!wI¹L¿ìŸÜßi‡ƒ?ÑÜ*7áïýeá±5mUNASNone?ï÷Ku""?Pö
l6ëž?QhýºØo?Pö
l6ë¢?ïþÊ?™ç?Qï'ÌùŸ?.ƒ\a{½?Qï'Ìùœ?ïzË£5E3?‰YÉõHx-?¦‹™WY™?‰YÉõHx,?ïý箢Ì+?)«ˆUaÈ?0Š鞨?)«ˆUaÇã4FGL J2147.4-3713?ïÎô9‰$òÀIðEwÙUÀ;=£_9MÀ<¥°<«'@Jô	Q¸Y@
© öÍ?ÔiÜÓ3?Ç(xY­ñ??ñÅÓé÷ÿ@)T ?ïK¤C@Çp¿á`<ZX¿ß£™!пå¸Úýgr¿ä°?bì^c¿ïÿþó…õUNASNone?ïþŠ®}ÑF?,õƒi)b?'U"ë®?,õƒi)aÕ?ïú7ë$™?b¾H¸–?G Sm™Éó?b¾H¸˜?ï˜S#†39?ƒêþ~l¶?‰ë7s1Á?ƒêþ~l¶Ž?ïâ'aÅ/?[SÈKQ¤V?mønž:ÐB?[SÈKQ¤U4FGL J2151.2-4034?ÞÑü=÷ÀI^xB0üøÀ:ó'÷¾èÞÀ<£›€#¦Î@Ö7"¦˜?ýŽ]%u?à.ªØ†>s?ÊÖ¬Š2é?óŽR
}?üɇ5=úb¿é¹j"Ù5?ÑJ?f9¿æ(C ¾¦ï¿Ò<Š?3œ¿ìòs_ž <¿ïîövÛUNASNone?ïàÁX?r_kV8±?o>êéú§ò?r_kV8±?ïÛ)áǤ'?ˆ*€(7€?rk-¾ž?ˆ*€(7€?î‰jù
–?˜è®ž6S³?§oyPo& ?˜è®ž6S²?ïz¢Ÿ¦uû?Q¹Äs?«¬1@§?Q¹Äs4FGL J2152.0+4718c?ïþƒVÃÀF¶¿DNÀ9®	SeØ¢À;À*zýÍ @öê5hl¦@
Þp?Á—ZúøY?Àˆb½Þ?ùÅށ*7@ՐÒÇñ?ík»9ýR¿Ý]Õ¾bü¥¿å {jÚin¿è>25r
¿è$SN[®¿âþ_
UNASNone ?ît6-z£?¬pB¾×4?¨¼—
(U×?¬pB¾×3?ï!B³à"?©kŠxO´?›×©ƒý
œ?©kŠxO´?ìŠcu¿Ñ?«Yܼv'?»¬äRIv?«Yܼv"?ì™I‹5v£?ŸÜ,¦ÀDù?»5³¦TJî?ŸÜ,¦ÀDù4FGL J2152.5-0607?éhó˜RÀEP|àP7À:ÎØÿ
6»À<Yÿu6@^X(`t@MYŸ®†'?Áí¤ž/€v¿»¾[T9"?ôáQ¿tè@ ÷TX?ïó×Ûôˆ¿é¾ÃŸ§z®¿é=²GæHŸ¿âçØVmÊß¿ïûDgõ?ïç!ý€É¿UNASNone?ïû¦·0•Ã?O`h¥[Ue?Ae#=¨öð?O`h¥[Ub?ï€KtÑ®?¢9äʶ"/?í"˔}ü?¢9äʶ"/?ï¤ni?'zùÏ¥#Þ?†äe˜¾Ë?'zùÏ¥#ß?ï½UËXÙ[?w,d¥l?€ª)É©/?w,d¥k4FGL J2157.8+7142c¿ï{ pº@*˜Þ 3çŽÀ:)öi~HÛÀ;©Â@ÐO@š6ªŒ1@;7T*?Ñs&hI•u?á©ñÖq'=@	ÂzÊÒ?ç¨"õ^¢‰?Ñàu =)¿áx+ŠÈE¿ê7\Wï«¿éò6H'iI¿í"bøóœD¿ïðà<ì™UNASNone ?ãW7æykÉ?Ձ›mÓ?ÙQ3
(o?Ձ›mÓ?оÒԴ̈?ӁûuG½˜?砖•¥™¼?ӁûuG½˜?Ûëí{†öÃ?µýގŸ$æ?â
	B<" ?µýގŸ$æ?2[ŠaÁ?|´‰!äÙ?ï‹6'Öxú?|´‰!äÙ4FGL J2159.6-4620?ï&Ò:Xe"ÀI=žÇÀ:—õL¼À<rÙ	1µ@!)n'E?úN¿ÓÀ?Ãæ[L
?²ÓF¹wÛY?ðî¸Ê·H×@5Ä:, Å?ïç3€`°¿ëõðý®—¿†4›¾¶¿ÒÓ¿ÿ4¿Ý?R[§¿×–ž<–‰DUNASNone?ïÿ}Hä?ç§æ«éá?Vãn]Û?ç§æ«é›?ïýó"äô?JíSFº˜?0fïØ[0?JíSFº?ïø¥'ë£ü?]ê<c¤?Mi¸QpÅ?]ê<c­?ïöG^&a?DwAÈF ;?SõqC³=Æ?DwAÈF =4FGL J2201.0-6928?åÁ<"%ÀD†Š›ÏÔ¿À:"›¯ôOÀ<n¼‡k @ö×?–@Uن³U?ÂD²w$K?×p"[<Ò@1êÝY@t^ÅÞ)?ìh§¾öJu¿áþËí©¼'¿ßÂ^ß´[¿ãßbцoñ¿ïÿü¿ÙŸC¿ïÿà‡êUNASNone3FGL J2200.0-6930?»Õ"_Å
`?¸%ß±ê»,?ì…Mt^T?¸%ß±ê»,?×èˆ:° ?ÓϳÜi›?ä»ñ⧰?ÓϳÜi›?À¡þëk€_?«˜Òë´b_?ë׀E%ç?«˜Òë´b_?Û»v«h–?¶ã®½ŽÅ?â"Dª}˵?¶ã®½ŽÅ4FGL J2203.3-5009?ïý%¬ïÂuÀIWÒòäÀ:©YÿOÖØÀ<j–gµò@êNÿ—z[@Ï8à^*?ΚÞ=7˜ô?×Õ¬$5¿U@Ê%£'·Õ@¯Lejh¿Þ/]›f£M¿ãØ®¸ϧ¿êu|N/7ü¿îCˆêí¿ïý¶CôK—?è"ËáëBUNASNone1FGL J2204.3-5017?ïÿ©Çœõ†?耊N4œ?ŽžqP?耊N4™?ïª(y'ëž?Ÿó'¦¹ÿô?…uᛅ«?Ÿó'¦¹ÿô?îü¿¶‡A+?'×݉R#`? 4—‹íH?'×݉R#a?ïŸ	¶ lå?|E|{v›?ˆ='wäƯ?|E|{v™4FGL J2205.0+0943?í
Ôð¸ÀA¯íúCþ]À;ÉvÖöò:À='õ`iÍ@ó{}"»@:a$Þ?Ûù©#Ð>Ç?ìlª]a/@RC;¾òï@ÞÄfKäZ?ïù"ù÷¨¿á'åÞÊm¿Îª9º`äq¿â'N
ˆ¿ð?î)‰¡ÑUNASNone?î(¶`?³ ¾Â}?­tŸO®©ù?³ ¾Â~?ë0Š¿²×?ÌtÍ`?Ã=Õ4¡Í?ÌtÍ`?çJé¯ðÔ?µUCf×¼¦?Ñj-î W?µUCf×¼¦?èEå<?ºÆ•5?Îë»èkë
?ºÆ•64FGL J2205.8-8254c?ê[Àçì›\À@+L`RPÀ:·ìj÷ÆÀ;ŸÌiiP@Y7žR@Ì}´'m?È.ªb?ªË¡~•\H?àV<'gMí?ø:*¨öü¿ëÿ!HO$+?¾™‹¬Æòî¿ì¨ X6¿ãÚ«'!ü¿ïþ/ ¬ˆ_¿àò«ÿ!Þ¢UNASNone0?ï®ýċŸ?'gä&ÁG¥?"@ŽÝN?'gä&ÁG¥?îÒý	^i¢?²#pñÇ@(?¢Ð/jeñ?²#pñÇ@(?ëÔHÑ1?©µ˜ÕBYï?Á¼®Ü»;é?©µ˜ÕBYï?ìÈá¼x?§$ü0çøÀ?¹¸÷Ò|B?§$ü0çøÀ4FGL J2207.1+2222?©
qñ ²€À:‹…ƒb°À;EL¢pñÀ<¤«ë«µ%@!/A0vëD?üãÙßö?ÌÕl®ì?®4'$D"?äfwŸ@B{pcÀ?ïùß?>¬¿à;×|S7µ¿ß:â
¿ÚG_:":½¿ØA«0šÒ¿äؼßï¿@UNASNone?ïÿ¯&Öw7?Øúî.á?6Jb23E?Øúî.;?ïþh/£+"?Q'']Ӏ)?)}ÍMäw?Q'']Ӏ(?ï÷kkÛ¶?_@¹Á0ò«?Q))ÜH'9?_@¹Á0ò´?ïø]U¢X°?<|}~P¿e?NŠ©v@j?<|}~P¿m4FGL J2208.4+6443e?ïdþû©–T@—Óºý—À8ꈟvRÀ:þNôYÚ@
¹Ø©Nî@ǝZï9ß?«z}þDN?Ê(dM1Œ@)'^aµ'@D¼(?ÏÝ5$Ïî¿ßi<x¬9¿ãjMT¿æ;5`4>¿ìŠþ_kö¿ïÿøsCÄ{UNASNone3FGL J2206.5+6451?·B!‡TÃ??»5ÍZÕë?í»Ïg™?»5ÍZÕë?ô£½‹z!?«óqsðWœ?ïˆ-q	Ò?«óqsðWœ?ύh+ÝbL?¹ äòa?è¥õ§m?¹ äòa?œru¾Ö+?‡ !"Íó?ï"lR	N?‡ !"Íó4FGL J2209.2+3710¿éu÷ËÝÀ.…yRژÀ:¸dàTÀ<D»ñ³6@êkñÕ¥@a
¿cí?Ƕ5?Ìt?Óóm_ÿÄò@õ*Ÿû ?ûãq#®°Ø?ïçz,ìÈ¿æàyó$÷¿ìܸÓÅ¿è]æe$G¿ïéºy
2¿èt¡B‡NUNASNone3FGL J2209.0+3652?è ZªÏV?ÉmnmV(?Í~•TÚª?ÉmnmV(?ã'(Ûhô¸?ԐìUç'?Ù±®I.?ԐìUç'?äíWö-£?·Ýii±‰?Ö%P¤¹Ú?·Ýii±‰?Ó'葊3?¶—L·?æ}ì·:æ?¶—L¶4FGL J2210.2+5919¿ïüëx@
¶ÿÛíÒÀ9r)=æë\À;íÂÚ@l—ù±\Y@´¯Ÿ•\?Îpc?jy?Ï陌- @Ž_f—äŽ@·ètH&_¿ééÞöšüp?È#Á{4ÿ'¿å×<Èk.¿ëÚß_ ¡á¿äʝþ-B¿ïþé6ßUNASNone3FGL J2210.1+5925?Ý(yËMµâ?Ð+ʘài?ákÃY%?Ð+ʘài?ÂH³1œ¤´?ȶÉхo?ëmÓ3˜ÖÔ?ȶÉхo?ØØ)–ec?»ÿÀ±í"É?ã"ë4ÍN|?»ÿÀ±í"Ê?ÖW³¿'»Ê?¾¿}¯?äÔ& 7"?¾¿}¯4FGL J2210.2+1624?äî¾ß*K1À?€6†¤ÊOÀ:ë 8ÛêÀ<e¶ü@ôMãÕ@Ñ=?%¯½?ÍFž6€?"i:£ŒY?À+Ëö8+@0w±èDø?êð
¿0W¿ìÿÒ]°¿Þ^úâ3ç8¿ç›Þ¸‡›j¿Ú«žê;r¿ïý©^2»>UNASNone?ïõhjVR'?R—ó³%?U/+SZۉ?R—ó³?ïý3 #ދ?Uá"V¯€³?6bþᨲ?Uá"V¯€ª?ï–ÈñEë|?…͈Ǘ©?ŠMî… é?…͈Ǘ§?ïñAgÉ?K—äª?]}1þxí\?K—äªý4FGL J2211.9-2924?çb_\h!ÀK|]¥qÀ;X°ô)2À<Ìõ¢®ì@ºò°Œ$?û'SÚr§½?Öã܉Ù2?É_ÃõbÃ?ò¹K{(•J@{ëöD?ïÿ|'1ž?¤Gò\ÿ4~¿è?k*M±¿»	<¿¤¿ä<~`ƒ#¿ä§f pbêUNASNone?ïÿ
D'2R?T¯µiÏ?Wo¹µÇ´?T¯µiÀ?ïýxÃK%œ?Q™v¿Z'?49å¦Ó#v?Q™v¿Z$?ïªB	TKÃ?ƒuól.Ì=?…o}ªív?ƒuól.Ì>?ïöùöë'º?B¹ÂBDÏ?R)°‹\?B¹ÂBDÅ4FGL J2212.4+0708?îG»ÆQ[ÑÀC=lß&k¥À9ù틉5žÀ<'÷‹½8@A•Ò¯`@Äô@¯¹?¿: 8ˆ÷?àÔ=ÿêÜW@ñüLY@DeÀN9I¿é›¸øÚqÑ?Å¢7"/ü¿Þ€Ç%CŽ¿å˜Ôýó¶F¿îŠ4¡È<D¿ïóðÈT˜UNASNone3FGL J2212.5+0703?\¸Å.ž6?`Êå½}ÞO?ïñ£h°å?`Êå½}ÞO?žÚî˜ó~¼?²Ž‹a›(?ï	(‹8d
?²Ž‹a›(?j7?€¹NK?ï|¯¾C€?€¹NK?ÝÌm®áÅ?}õù&¦K?ÎIDy?}õù&¦J4FGL J2218.5+6822¿í‡¹gŒ]@#"Âß
A1À:ôنïrêÀ<Xu²3ÄS@ È®Õ@
â?þç,yێ1?ÏhMÇ3/Ø?Ï`•ÁóªÝ?û>[ØÉ@Tdù7¿æ9€ô¿ïÕ E…EO?ïÿat¿ãsBí»¿å{:3µ¿âÚ!I%ã¿UNASNone?ïü4Ï[ãÑ?A.QÆ[8Ì?>Y… áw>?A.QÆ[8Ì?ïùŸ¦Îid?gÛ°^m?IdÆZkà?gÛ°^m?ï'áiµ?‡3SÂnô?‹G¹~e'?‡3SÂn÷?ïؓ^Џ?eH÷žÄv?s¶7З¸š?eH÷žÄr4FGL J2218.8+4736¿è¤–óºp/À¬'ªÀ:ã5ï¦À<À®	"&¹@©¿©MÂ?ÿDâ–?Ë0‹£Œ·‰?ãæÀhæH@ªèžºjÊ?ÿ½Qӟ¿ëø˞#—	?ï͚R&=¿Óý‰ƒ!7¿âȅufοïUŠáoò?¦M®ß{ûúUNASNone?»Ù£ÈÊT©?µð`áp?섈æµj?µð`áp?È[ø-(Iè?ÌÛ¦ðÎO?ééôµí…?ÌÛ¦ðÎP?´ÌÐÙ.W€?£Åé¾ >?ífeäÚ5?£Åé¾ >?Ç£Jn3"?©ÙŽoV•?ê8-ds7?©ÙŽoV•4FGL J2219.4+3229?́—TàÀ4F¸Ø#B$À;r:âTÀ<ªXÆj²ü@!i´6Rø?üÊáö)½i?ҚÂïH£?¿Šk©F_á?òs§Ös?@å"…à¿ïþtDuzÖ?ïõ´bÕ¤?Ý:ÌÏ€¿äTíB83ﻥ°Bi¾¿Ùœ	€²BUNASNone?ïþ»×BP?%ø?!?$G‹Û'?%ø??ïýÚ(Õ?T
w.¦î?1.¿ÇyY?T
w.¦í?ïӝ­çæ3?w]%¦"›·?v1)æ9?w]%¦"›³?ïöYÙ)-?GÞ4bÐ?SMÀM­¦Î?GÞ4bÍ4FGL J2219.7-6837?ÔVLYÀEqûçl‹DÀ:ãsê³g¡À=§"ïQ@¶`Ï£–É?øvd«{Cm?ʶI'¼1Ÿ?åU2âUu'@	­Ý|é?ûÚý‡TȄ?Öž 'ðÙ¿ÔÇå</[7¿´•M.±ï¿àµFÓù縿ëљ_â隿ïo)­¯PUNASNone3FGL J2220.6-6833?ÄiÕ_eZ?½éc:ª?ê动&©z?½éc:ª?Ñ¿%ý© q?ÔÕ ÇuO?ç m+/È?ÔÕ ÇuO?ÉHÝkëbÄ?­ë%èý¼`?é­È¥'P?­ë%èý¼_?Ð;…®ï?¹."†B?çâ{½(ÿ‰?¹."†B4FGL J2220.8+6319?ï´¨+µ	@ßßã*dÀ9Қl'qÀ;%/<-®@` §@~Ú4"\?¿7¢®–*ú?Öík¾?j@»øáþ9?ÿS¢F'^ã?Ó¬îàóË>¿×>l'	Z¿èDîs¿é†ýY¿í'T~1‰:¿ïÿ΁ز´UNASNone3FGL J2221.7+6318?ŒèWŒÊy?—ݧ~[Š|?ïŒ_¦¡ÌÖ?—ݧ~[Š}?‰¶r´JŸs? nØˈ'?ï™&5.Ճ? nØˈ'?Ây+}?¯K(ŽÕEÇ?ëaµ>::!?¯K(ŽÕEÆ?hS¯Y]ñ?SLÁô™¿?ïç¬P¦¢?SLÁô™¿4FGL J2222.1-3907¿àêJé՜ÀLfѝìåqÀ;»HCe°^À='ÌÍ£Œ@ /ƒ)j²@
­¾Ìf?ϳŔÊ'?"½l˜À¼Ú?É B€-6ð?ó—8¦d®*¿îñù@É?騣ÂèG}¿ê^°Å/Iš¿Ð¨n^,†¿ÑÌ1|#çç¿ïýëóفUNASNone?ïøáéz5?[kNyPS¸?LxZ·+C?[kNyPSµ?ïèp—yjÙ?€Oч&Ø¡?gh†•&M?€Oч&؟?ï¡°¤ì¹Ç?‡w´Òy
h?‡"ÖÄюD?‡w´Òy
g?ï×­9Cl?g°]Ü«?t)rc^J|?g°]ܪ4FGL J2222.9+1507¿ê±ê쐬ÀA<fÙ×À;]`—Ì:À<¬ŠLõ|@éd'%ÜÞ?ÿ'ˆ˜ÀUÆ?ßuaù±?µVóרî?Úèpa'ëO?ÿßY´Ò/7¿ë°ýñ‡í¿å'¯Šœ¦"¿ç·ëÿ—û4¿Åóµ™ÕT¿å³ÿvmE¿Õ—®\õ#ƒUNASNone?ïþâC9ù?&ĵnZ‡?!ÞûÌ`oã?&ĵnZg?ïür-ì ?[-.äU\¦?<nžÿ‹?[-.äU\¨?ïÌ°Ð]?‡ÉÀäA?y÷§—Ñu¹?‡ÉÀäC?ïöO)?FÊõôÙ~†?Sýaÿ­ïü?FÊõôÙ~~4FGL J2223.0+2704?ÃEvš¿yÀ9£œQÚ¾À;0<{±QFÀ<‰SŒo¬@=:ªËÆ?ü««u+%?àQ>¡{eQ?Û…;=ð?û»'øme@¦NTvÏÀ?ïñªÒ§a¿àç}mi¿à͒?2D÷¿Ýi'z™#R¿ïÿüoQÇs?îû¬ž¯7UNASNone?ïþöèz–?&s£—f»Q? Ÿ±xV¨?&s£—f»A?ïý+Qáï5?[×c)oˆ?6¥pð†Qõ?[×c)oŽ?îÉé¶ÔyÛ?–vKèwã\?£ad'¸bW?–vKèwã[?ïñç@Eq?Pë"ªX|?\1uÒ¦?Pë"ªXv4FGL J2225.8-0804?¤âÔ¸¬ÕÀITÃóà7
À:Õô_¸Í<À<xÀ²¤-@ z@Ï~?ýæp­E£?ÈëæB"¥?À›Æ…
ƒ?ö×#gäè@ö/ýV'¿ïÿ¤Dî?ïËŽz\¿ÚÞ߉gó.¿Ý6çˆ9õſَÁ#vQÁ¿ãU§11Ñ3UNASNone?ïý24"ºµ?3i—ϼª•?6n[Z*V²?3i—ϼª«?ïü• X÷‡?VŒZ'Nž?;Rý8Cő?VŒZ'N›?ïí.GÈ?ieiù8FÄ?bÑì¸7åd?ieiù8FÌ?ïàê"©ª?_ÛÿtqÀ?oláVUK?_ÛÿtqÁ4FGL J2227.1+6455¿€ƒ†]–Ùd@Õw–9'ÉÀ9ÔyìU(QÀ;FT$D'ç@ß}­Õx@	Zìeˆ?ã…Üî'ÿú?ՀW¾­Ð2@'}ke©¨@¥ºIg}¿ëÓ>€ï)?ïô ~$É
¿é'‡ÂÀð¿ì(ԟÿå(¿Ô$ÀS퓿磢AˆáUNASNone?ߒ@µ:m¯?Õý夸±?à6ߥbÉ)?Õý夸±?ÝN¿7/ƒ?ÔºtÝ­äÍ?áX dxh>?ÔºtÝ­äÍ?ܧý~üè?½w*CUš›?á¬7À‹?½w*CUš›?؟`†cáR?ÆÌ,{Ž"?ã°O¼ÎV?ÆÌ,{Ž"4FGL J2229.2+6421c?¸"<¥îÆ@v2~ØM4À9÷Å&p­À;k3—Ý÷@#Ü­ ¡@Ÿ!Í°"?Í,õ×]?¸'à™³Dæ?ñ`Ñ·Xâ@FŒªó´?ïÉ©—=žÇ¿æbڻοë$Äpù¿Ûg則¿ë¨ø5u¿Ý¨;¾/áUNASNone ?ï·>¹ø?‡èµÖPëG?'0{}т?‡èµÖPëG?ï/ÖÂÇ\C?²<³ »=?š'§wŸ?²<³ »=?îÊ[$'û?¡9ÃèÉ$?¯sZM·ÐY?¡9ÃèÉ$?ï˜Y‹@?…­vP ‹Ö?œŒôΗÿÁ?…­vP ‹Õ4FGL J2233.3+6530c¿èš+ìL·^@yw JÃÀ9¸3¡<]À;U¡ZX;*@¹–J@6>Ðö'9?Ä×ñXP?Òc^߉gó@Gª%Øם@ÒÒË>'¿ÕÖA?»VÙ¿áÞó?þѿ檀¥+ô¿ç9¾'‡.]¿ïÿþªJl¿ïÖ¯¤ÚUNASNone$?Éß·ðjw°?ÃäIjçp?éˆåb?ÃäIjçp?Â?ã°0q?Å)–úr÷_?ëpùóã?Å)–úr÷_?Ð!ݲÙɑ?²XNõµÄ?çï&"7?²XNõµÃ?˝ô!ˆb?­>ïó×<?é'÷»ç?­>ïó×=4FGL J2234.2-4156¿àU¯M˜ÀM2ÃC·õÀ:¡HËJìÀ<ªº€™îS@etùÒ?þ&~3⅜?ÁÛY£ï?¿5£ÐÕ#?ý'ßäÅù@
šZ±ý=®?ïÄÞ˜¯¿ÙÖä¾0&ä¿ÝPd[õP¿Ý_Z©™Â¿ã7PcÅ¢6¿ä©N½þ'äUNASNone?ïý÷çï±î?.‡ï×DÃ?0@À'p›¾?.‡ï×DÂ×?ïþ.àào?G·äôߙç?-ÿ1ùØ?G·äôߙä?ïóé5½\?cµp76Ûc?YÊ-"…H?cµp76Ûn?ïüsQ?*ŒÑð%?;ôgõwÔ+?*ŒÑðJ4FGL J2234.8-2610¿¾eÙâ¶,ÀMǝØ'tÀ;~õÒ-_À<óPúÄW@ '®K½@Jv¾£>^?ËJ´C¾ñ˜?'úu7˯}?ÇnÕö— ˜@.$kSŽ¿ÍïßáÒmv¿à1ǂàð¿Â°…ƒâù	¿â$`JmŒ¿ïþÛ"31?ïø'K‰ÁUNASNone?ïüǯðœX?8Ó(/e?9€{B²?8Ó(/e'?ïüq·wŸÎ?Xì±G%(?<rDCX?Xì±G%'?ïZž/Øü?Tñi¾îó?"¬:ðu?Tñi¾îô?ïû)K°^?;f©Z÷.h?C[¦Ñ>†Ï?;f©Z÷.X4FGL J2236.9+1839¿àµ²)›áÀ@æ$Ý/ À;+k¾"üÀ<²³	­'ì@ ¦·ÙÁf?ú»iGÂ6q?ÛGaS.Ô?Շ­¾êŒ?÷æê…Dwÿ@'Q8×·â¿ìÛ;$™<}¿ÔW­Ñ_ſ堕 ãû=¿Ö3ÍA¼¸Ø¿ÝÜæ ]ƒ¿ï÷mõ¦àªUNASNone?ïøܝ;ª?^‹Ž*¢˜Í?O"‹\Í?^‹Ž*¢˜Ï?ïü%ÔsZ-?d'Ø#7
?>Ñ\e."Œ?d'Ø#7?ï­®ʑ?'ŠÇÏp¥ ?""}?M[±?'ŠÇÏp¥"?ïßy½ T?c(\¾œ?pC!/õV?c(\¾œ4FGL J2237.2-6726?ïÜXã[Ù±ÀFq€AÀ;¼Ì¤‰À<Ó+—]7@ 3M«?ÿŸMR™*?ÏäÄeJ2?¹ü*9?Á")Ǥš@÷Ÿúêü?å).—ÂÿÄ¿âæŽà3·¿âoÒá8ꂿÜ)•»»¿Ú½ÒÉfÿ¿êKWÇýUNASNone?ïÿ£žsµ?a̯·?c½Ü0?aÌ°?ïþ–ZΕD?D÷èdnÈ?&šS«ÁÛ?D÷èdnÏ?ïù^1±Z?[ۑàkÖê?J‡9;Š–±?[ۑàkÖá?ïýÔ6Ô¦ô? øÀ\º?1^IZÈf5? øÀ\´4FGL J2237.6-5126?ìtMÛgÀK"DAxpTÀ:ÏfhæÀ<bÜ¢c@kíR@…c¯˜?Ó4Ú–Ž¢?ÙPê°£?ø
e~ßÙð@äÀ»!ª?íÁI̽¿èC}ÎaøC¿ï#¤FÞâ¿àhŸ[zz¿äk¼|±¿ï³¹€iÇÅUNASNone?ïýì€DÑ)?:^ó>¨I.?0›ýÙv»‰?:^ó>¨I?ïÝ©î/2??‡r¬'N?q+èfà?‡r¬'N?îÂÈæöIT?—N|úÓæ
?£Óq›j¾?—N|úÓæ
?ïÜãsóòZ?f¸J÷R•?qŽFÓ?f¸J÷R•4FGL J2240.3-5241¿Æb5çT_ÀK[I@»±òÀ9Ç]b±¦À;',kûÒ@ Ã-nÎõ@4M:'£?³ÈJ±ÿì࿦nJáO»ª?õöÁ]-Á@eÎà"j
?áh æ)•%¿ëšJ~©SK?›"*zä¿åYa/ÅÀi¿àÖÔBaúF¿à¡ýì)‰fUNASNone?ïóÖ7Xwç?WV.yÊ?XS'O0ß?WV.yÎ?ïýþ"?O¸Ï¥½¦?7׀ßy?O¸Ï¥½¦?ï£Òôvä?‡bmp´	?‡BûbG?‡bmp´	?ïҖõò:??g°Ã|Œ?v´…âà`?g°Ã|‹4FGL J2241.2+4303?¹&]\À+dî
öÀ;µ^>JÀ<Ô6>@lf EoÌ@øBf¬ÝC?Õ5¯D%ɾ?ïÿÜ>Y×ã@R%1ðÃ?æ -Š&ßé¿êŒëÖ}O·?k`ñ²_¿áæ͓œ*¿ït¸¤ Ü¿ïñÓíR~R?á 1ί%UNASNone?è†5Ôf?Ò•Ù3½?Íç+Ãä®h?Ò•Ù3½?Ìò0¦\Fì?Ӱс¡Jó?èÃsÖhîE?Ӱс¡Jó?Ó)Pêè-?³é
šP%??ætëWŠ‹é?³é
šP%??a?ðÃRÐ7?Pí¸µ0î?ïîÀ<­/?Pí¸µ0ï4FGL J2241.4-8327?æÀôž^ÖoÀ@J^	}À:°Ù(û¡ÌÀ<…Ål†;@ýTÔî"?ÿ‡7|n¨?Êd_:£?ÛÍó}抹@Ê%ïúÏ@n½:2«Ï¿ëY@¹À¿Åù'¾8ß¿ÝÔ>{eÑì¿Þ²	Ò癿îåvå¿ï裝SqUNASNone3FGL J2237.5-8326?êÂ'»mÇ?Á4FT¼?Ä÷ÝõHæ?Á4FT¼?ê	rèÂu?Ð
¬Žæ?ÇÚ4]øö-?Ð
¬Žæ?Ù½ìšéC?½ÀüM?ã!	²‹^}?½ÀüM?ëþ?©Í?¨î™DºVª?À¿©XÎ?¨î™DºVª4FGL J2245.8-4148¿ïùâ¡hLÊÀN=þ!ÙnœÀ;"E	Œ³À<ïð‹î¶,@"Y‡°¸ð?þ'Ù--_µ?ÓJ"ä(3%?Ï8ùÜ$ƒ˜?÷çESÇ'q@_Î$1?Ò¬cû¿äì¶wò¿¾'¡T£ñ¿å}Ä@âl¿á°'¿ŠÄë¿ïøž;ê½UNASNone?ïð^{Õ?nٌ¾l"m?_ÉCÉTõ?nٌ¾l"i?ïø(Þú©¸?j¬ýÕn\?O\"Y«?j¬ýÕnX?ï
µ£¯Û?'L¦I»½?œIKŠ¢?'L¦I»À?wlY­?n'ôsW‰?€b$é"×?n'ôsW‹4FGL J2247.7-5857?±G™.ÙÀIÔÖõD»À:Ñ×ÙôÓÀ<&0ì1@£Ð3ç¹@¶½2%?½5 á6'7¿¯©¬â Æõ?ñ7jК¸@"'[d±?ïüL·h·y¿èMW¡§…¿éHÆÆ"¿àMÉåX4¿éóaáòN¿ïÿ-½R†`UNASNone?ïôÝêXI=?kÎ!¢ìË?VD+Omƒÿ?kÎ!¢ìÍ?ïój'ÝÉ?n—ÍZµ?Y*á°Dn?n—ÍZµ?ï¼cJ-,
?y'™˜Û?€ç-t´ý}?y'™˜Ú?ïÛ¤¨ûÝ?^˳Žiã?ry­«')?^˳Žiå4FGL J2249.4+6222¿émœ u''@C±Ã\
ÃÀ9±úã`	À;ü}"€U@;ڌ(õ@¬{­?ÓÈD½IL$?ÇÉD6¶Ë?þzŽÜ§5d?á>ÚJ± –?ï­Ê¾­	¿Ü3Յ2à¿ëÝü›Çq¿æT7ûr¿ì©c`Íu>¿ïöQ*"ÿUNASNone?åæÖÕ^?ÑTÝÞüöÂ?Õô2SÜUD?ÑTÝÞüöÂ?Ö¢I>¬?֚Zÿá8¨?ä®Ûqà©ø?֚Zÿá8©?áæ@ú"??º¯F8â?Ü3Ö
÷?º¯F8â?"zܳVTO?ƒãˆ[ø?ï\)eM^?ƒãˆ[ø4FGL J2250.5+3305?ʬ­ZÂÉÀ7H`RP/À:<GËp¬;À<cþcGÍõ@cá4¸ÄW@ϑE7A¶?ÂBˁž%E?ãóÞ>d>Ä@f<ù…'@çâû{9?ÙZ…<ji€¿'Š;¾Ù*d¿âÖV¹J9¿ë²'LÃýñ¿ïÿd™ÝŒ8¿ÞBÛ\\¢BUNASNone3FGL J2250.6+3308?fAšcHßê?døL'?ïé¾eœ· ?døL&?˜[e¼7É?¡'‰òºÙ«?ï=$×
B?¡'‰òºÙ«?¤YdK51?–o&™Žy?î¾Êi»L¬?–o&™Ž{?•êBŒˆ?€rfNG?ïP­ëŸ'd?€rfNG4FGL J2250.6+5809?èé/êc¤¿ðûx–ê'°À:§¢>ƒÉNÀ<	ɓ\i@!'8úóPÅ?õM
À¿?ß}~á‡o?ÝÏ`cò@I][û©Y?óüûhÁŠy?íÝ®ˆ*Ü¿ïù¦êºô]?îVÃ[4=¿Ü«›úœê¿Û1s?'½¿ïã¡ìõ6UNASNone?ïvP#I|¥?œ¶"‰-*²?'5û–Ðk_?œ¶"‰-*²?î
?×½äÿ?ÅQ.2Ò?¯\"!°?ÅQ.2Ò?ì\»N~?©|/_ß—?½#•Œ?©|/_ß—?é´C<;?¹¬ýE:?É.óÇÐ?¹¬ýE:ž4FGL J2255.4-3252?íõ¹/VãÀP"ÊÕ{ÈÀ:ÎCr‰ŠÀ<¤é½ž[ @ÙIŠ8@¡ƒræ§?ÐYkáÐj?ЂƒÓ^·E?þV'Tà@ÙE¡Iç*¿ãÅâB)ñ¿Î	{(ë1¿â­×>?׿æì¶!9¶…¿ê`üßåy¿ïÌvÀü‰ÿUNASNone?ïΎ؊ßþ?|ôrã·¶ˆ?x¸"ºÉ?|ôrã·¶‡?ïõf?·?lËý\é²?UÉÏ3€'î?lËý\é²?íì ¼d5?ŸËF,HÞt?°žÿÊÞZ?ŸËF,HÞq?ïÎOCoæh?h>ORF?xØ^HËT?h>ORF4FGL J2256.5+6212c¿ïÿ2–ýÂ@ "S.{>À9r« ªšÀ:íև`±ñ@R°ŽES@Äg£}?ÐD~Ÿ˜6B?Þ¸AíHm@[輜$?ñÌGVUÍ¿æmE}¸'ƒ¿«iü"0·ê¿æÔS©Ë@¿íüŠ_iòã¿é!	?nÕÌ?Åáœ}#Â'UNASNone2FGL J2257.5+6222c(?Ê÷¦VŸ\?Оq£ã?éB:ÖjX)?Оq£ã?Ѕ¥'ƒÚ?ϧ™:§³L?êÛޖ¶	?ϧ™:§³L?Î˼Í,¸?´E‹"G?èM̾4Ò?´E‹"G?"® Žïšy?"…i^ûK?ïbŽûˆƒ,?"…i^ûK4FGL J2303.9+5554?Ãðè4nÀàÒ=OèÀ:Åc®ünÀ<^UªV€@!¸_õ‰Ÿ?üŠ"C"?ÈÁêAÞG?Åq!Àŧ?ü£mWò/@]Ñ8Â>¿ïÿø]ˆò¿¼ÙÃUU?ïÿÎÿYg¿Í7IWâ¿þ¿éÈ}ýܺ+?ÂJÆüÔ'UNASNone3FGL J2303.7+5555?ïÌ£:Ôò?|™¢øE¡?y®b•ò†ø?|™¢øE¡?ïáÏ>j,?˜"*–sr{?n0Á•çÓô?˜"*–srz?îØÏ{c>n?–¼Òˆ¬á?¢sIÌ?–¼Òˆ¬ß?î¿çW¶>?—"ÛFï¡Z?¤Š"—ì?—"ÛFï¡Z4FGL J2304.0+5406e?è²RlnÀXàkæÀ8›Òß5…À:äk篧"@#7›!Ùï?ü-SaÅ?µpb=·Æ€?Ï>;¤ò@"è‹+B?þ§mrU¿ïÿêњ'ç?ïÿ› 'V‡¿ÜÐæ7
¿ºWìPӿفà•V"¿»?#@÷ÁîUNASNone3FGL J2309.0+5428?íøö¼r¤?¬|JŒÐ?°8Jkzã?¬|JŒÐ?ÑWìYÈ
?Ԙ0è²L?çT	Ówú?Ԙ0è²L?é{áã.€?±²‡Û~†,?ÊxsÿF?±²‡Û~†,?¿ï7Lƒµ³?´ð-NnCã?ìo‰J?´ð-NnCã4FGL J2306.6+0940¿ïÌU&õŒ2ÀF£sÀÁüÀ;)Î悀xÀ<†\<@øï@2gà9@‹ƒVa6?Ë'4!o¼P?¨U:Þ¼þ?Û%l 9±R?û:µÃ›Ë£?îêI¥Ò?ê©érõÁ¿égÃd™¿ãôJ?>YW¿ßJDÝ)¼<¿ïÿ!ž5_³UNASNone?ïîLiò?c¹%†)æJ?a³â–ë
ç?c¹%†)æI?ïÍ¢WdD?"zù7ËÌÍ?y.Ô}MÝê?"zù7ËÌÍ?ïEÂÅ…I?ž"Äs<?—G§]VÓ?ž"Äs9?ï`j;G@y?"YB¦\ŠW?"ò¸—ðø?"YB¦\ŠW4FGL J2311.6-4427?ᆲª€VrÀOǛÜiøÂÀ;@­
ê¤NÀ<¨¯3+¦@TjX¹T @9×wJº8?Ô.]¶i‰?¼¸—
ÉÅ?éŽ_tÝÛ@¶ø¥Ò?âØ"ð½¿é³hb?_¿år¡L$œ¿ÝTŸÿå(
¿åly¥ÞKz¿ðUNASNone?ïþà—¾ês?!ûÞ(°?!ö"XÛú?!ûÞ(°á?ïð ñªô?uJËÃâã¯?^¾«öD?uJËÃâã¯?ïä¹Rº4f?r"ùÊó_"?kF­E˙›?r"ùÊó_?ïæ©Ýg½&?X>ҞšÕ?iV"˜BÙü?X>ҞšÎ4FGL J2312.4+8253?íÀv£)݅@4£ èBtÀ:œZxòZ%À<EÇwù5á@̎²µÊR@½aÀxi?Ð6>"þ?Ôq³/lÕ@ã
ù½Æ @77F¾*s?î8Çâ'@¸¿ãÚ¨ÝÚ;J¿êšÂ
¬¿íÚ)vñÎå¿ïÉ4â_Ü	¿é8âií¤UNASNone?t¾u?®¡÷ê0ÓÞ?¦æW(´¸?®¡÷ê0ÓÞ?âAèUS}?ÒM¼…Ô?Û|/UYý?ÒM¼…Ô?ê»8‡mAF?­iæp¾¢?ÅâJúä?­iæp¾¢?å¤TY'Ó‡?µDÐöX/«?Ô·WLúXô?µDÐöX/«4FGL J2313.4+5947¿âù	1íA]¿è«ûèCKÀ:&†ZøtÀ;;ÌÛ…¯@ ³˜zµ¨Ä@‰~Jˆº?ƣ歰¿£$"3ÿ
?ÞÑ0ÿÒ2½?úî5r} ë?ïô`Å<µ"¿Þ• c!ãU¿è_øù{¿ç\¦>m£ò¿Ó4˜Žß#¿ë
Οµ½gUNASNone?ï°Þ?ÅX?€§¡JĜF?ƒÈp©ÿ‹?€§¡JĜF?îõ)¬WÙ]?¼Ur©<âÒ? ­e:'j.?¼Ur©<âÒ?î~R`Cõ?ž'xõ¶÷Ý?®xÙûÀ¯?ž'xõ¶÷Ý?îwÔ÷Ìx?˜=rÂ4Ì?¨'°ƒ>xˆ?˜=rÂ4Ì4FGL J2316.7-3144¿ÛîØ|AµpÀQ;27Š°ÉÀ;=•ôÉkÀ<Â"<jêZ@èák•O]@9þ¡[.û?Æ%]‡š"•¿±=èîÁi?è¹EÁ€=}?úˆÂ>SwÌ¿ãýž%ðU¿ì´R¿Ýñ¥U¿ßgk1|¿çŠ¢OοÕð?ÃdnUNASNone?ïó~<q?TBŽt¾bÞ?Yï†Å ?TBŽt¾bâ?ïÚºŸ…?…Ù`#]T?r¢òð0='?…Ù`#]V?ïžeòÂW²?"»9jª/¤?ˆfƒOj˜?"»9jª/£?ïÝoÀvß¼?`½
ˆáã?qHĐ"?`½
ˆáã4FGL J2316.8-2518?ßwHŽÔ­÷ÀQ/Ë>WS¤À;j@ºˆÀ<È)ösD@8bè,¤¤@7^nÔÊ@»·Þþþx?·Ç¡á^T@r»3rH¿ïûƒ¶?ߙС½6¿Ýåâþ"P¿åÏ\>oQr¿ïþ9 ²ýï?ïøª O€ÇUNASNone?ïù~Š­ ?QÔݲuóÚ?JÕKó`?QÔݲuóÔ?ïó[ÏEè'?u«®N¶*ó?YHat.Þ?u«®N¶*ô?îH
-&ƒ?¡cR/½&?«~/]-—Æ?¡cR/½&?ïü)tS0?Bµ´È1[?>´]gւÅ?Bµ´È1[4FGL J2317.7+2839?Ð1…V/ùÀ=ÜÏ|ªuŠÀ:j‰á•²À<hÇåÝ?@ [¡äì©6@'U»Gi?¹nlŒñ¿—E`dø0?àšf³"?ã@
Rí*eYK¿Õ·¼]éÀ¿ßôYĚ̿âa8ÿûοá+8'ŽºC¿ÞÇ¢@‡.³¿Ó\åGB	UNASNone?ïþm­EF˜?+qî²:ÖÛ?)%+«–—?+qî²:Ö¾?ïþÆ,ÿ'?BöDH;?#0߁?BöDH=?ïøòº{Ñ?aée_™b?L5œ»f?aée_™i?ïýêSqö?!£ñSó¸?0­c"p[¶?!£ñSó·›4FGL J2317.8+6140c?à›ø£(Iš?é˜c8´|tÀ:݉³r‰À;"•µŠé@"»ï¯Ð¾@Gz>Š?ÉÍ$`‡;?׺šÛŽ½@
À?`h?ôΨB¿ê½˜]ƒ¿±dS爺ϿÚÈ2¾ïŸ¿éÖð¸»¿é€Å§J¿ïÿþÐñUNASNone!?ÁѾ‰€«^?Ál—lS/?닐]ŸÕ)?Ál—lS/?Âܟ	j¡'?Îóƒoíiß?ëHØ=¥Wœ?Îóƒoíiß?Ï°™'^ô?±´Íz} ?èÙ¶(Bþ?±´Íz} ?²­v©"?—¯÷ %ß?íªQ?
Û¿?—¯÷ %ß4FGL J2318.6-3827?Éh¨ÜÿnªÀPâpdìé£À;٘áõ²À=Jb¹3@û‹¨jAè?ÿ@[ŠjQ­?Ø9Å^?ì¢E¥%¾Ö@šð{þ~ @Ñʽf'¿ïÿå=†ô&¿ÁPɆœ;à?ïú՞­«¿Þ$#á0±ú¿ìgs¬ ›¿ïý_ÂvíUNASNone3FGL J2318.6-3829?ï@þ¥4+?žÝ:0H?—ü€+Yzª?žÝ:0H?ïŠ{GO??¨ù6¿÷ðx?xa.,0?¨ù6¿÷ðx?ìRt@‰šU?¦ƒªrqM5?½l]û³-R?¦ƒªrqM5?ìÏÐì#Ž?¬]O¼.Xb?¹‡IxžãŒ?¬]O¼.Xb4FGL J2318.9+4151¿Ébá"½À1ŃùdoÀ;¿¦sœ°À<Ví½\ì@Ô¥Èüލ@™#²?ɖ÷¨Ãƒ"?®%{·?åcä
Öó—?þàUÓq+¼¿ïƒ"4?ïÅ(ÉL匿é$É®4[Q¿á@$³=¯Ž¿ëù—eâ²è?±qj{sé²UNASNone?ïƉÍ:ò?~a/ó6?|»bó‡?~a/ó5?ï¶[¬4{Z?™sšä:?'iòá)R?™sšä:?ïEÓ.?'_PÒo/b?œ÷^…š?È?'_PÒo/a?ï[ás¤gÜ?"{"ž»º?"ƒÑ‹sy?"{"ž»¹4FGL J2320.1-2440¿ï똛ç¨ÀQV灃ùÀ;75c'À<°Ô8í‡@"·ç7‡@'`}Y"?Áƒúuý]8¿µ)žŸgäÁ?óÁC|V'´@mÀÐj;2?æêŒÑ4;¿èÏ_žÌ'¿æ·Î8Ø¿åù˜¨)?µáVáRÈ¿ïÿÈb±UNASNone?ïú9Œ?BSþ«Ü¹¿?EùÃϖ§?BSþ«Ü¹´?ïý¹ÖM?Nh]zÜÕ¹?27™M—Á?Nh]zÜ՟?ïÕþØAá?wWÈ¥S9è?u"ý_J?wWÈ¥S9é?ïú5¤9È>?@;xqæ…?G)oßÜ?@;xqæ…4FGL J2320.2+0707?Üæî
ÀH _ZÙjjÀ;=®¸å;À<‰é'9Y@!
/ÿL%ó?ü¸âe+Ô?ÓÔR?´J*ñpE7?ãà÷?ò=æ*þ¿ìjœ&@‡?ïw·ÒiÅ¿Û~ž¡@W¿à؆¿L[£¿ÃÏ¥ïa¿ä­rÊ!÷¢UNASNone?ïýúE¸áš?4LÊQF?0-Ò8ó0ë?4LÊQG?ïÚ>£/?ˆº6÷P5À?rñàö.hs?ˆº6÷P5À?ïÎÅfμ>?|° :»?xL˜¡àç?|° :»?ït‡$܎ã?'+ÇVŽ¿?'odn#š?'+ÇVŽ¾4FGL J2321.9-4842¿ìvˆ&T$ÀO+Ê! áøÀ;'^±ŽÀ<™Dwÿ@ð³¿Õ˜?ÿÁ†}]"ñ?Ð
,8m.Ø?ºxîÍ?é¬ÖÝÇÆÔ@?X£Q?҇±d¼m.¿äÛ£ß¿ßfÙRí¿àìÒü'¶v¿â-«¿‹ñ¿íù> #ÌcUNASNone?ïþW "€?%tòvƒ"y?*†ýöÈ—?%tòvƒ"e?ïýö¬eé<?G¦ƒ+Kô?0JœÐ¶à?G¦ƒ+Kþ?ïï'än¼?j ñ+b?`ôn'CŸ?j ñ+b?ïñ‡‹;?Lc8Kô?]ñÞéŠ"?Lc8K 4FGL J2323.1+2040¿æš,"ÀBÑ|o½'=À:ÚýPùØÀ<kymª'†@¯ˆc'Iê@¥ÆÁ#?ÃõB6Ü5 ¿¢ðš1o
Õ?ádðD¡?ÿº°?£Y¿è7Ïᗊ¿Ú5ÅaŸ¿ç<lݣߙ¿áʓÒ}'¿Øx\2/ýõ¿çÝu&Ê;UNASNone?ïñšgÝÞ?`|Á1½¤?\üË0DCû?`|Á1½ ?ïù^!8¸?o™&iEÈ?K¾‡{#g?o™&iEÆ?ï½Ã2´¾"?|ÊBöêx½?€3RÐ[=?|ÊBöêx½?ïëñeˆ?T5Kð!M?düîšwí?T5Kð!R4FGL J2323.9+2519?Ä!rǁþEÀ@ºç¯·éÀ:Ï'`—À<‡ô9rè@¢@ÕXå?üqišÐ?àÆdÓ¿/?ڒòK—
?ü¸ŸÔF=Ò?õÑ-=û¹¿èz9¢õ¿äYÈ]ÒC.¿ãEgéel¿Úü•½Aœ¿ê¦k93þ4¿ïýwƒ–"UNASNone3FGL J2323.7+2523?ï͍ëb'/?‹L¸ß?y9
N¶è5?‹L¸á?ïPýˆ'¶?§áБngÅ?•àNü;	-?§áБngÅ?íê¡sžd?¡c㤳+Ø?³ªôcâ?¡c㤳+Ø?ìßF?ÿF?¥hßøÑ?¹ÎÏ?¥hßøÑ4FGL J2323.9+6219?ïÀƒ'Þ?ò"cښë©À:}Ñs$ºÊÀ;™®°'k@!!|o?@«j©Ø¬?ÖÙ¶Ÿä·O?µta%߸?ßÒèûV¢ú@®6Ñ?ïýä×Û¿î/¬*•ÕÀ¿È†ëA,¿ßu§·iŽ9¿â†=œBÁ¿àÄ(ï'µUNASNone?ïó…M)d´?nüQE6Kø?Xõe­6—Å?nüQE6Ký?ïž0T?®â~±vO?ˆx¸|3êù?®â~±vO?îŠO†ô?ê€ŸþÚo?§^ې¿?ê€ŸþÚp?ïy¨«ÕÃ?€+ìyÕ¯?Êêœ%G¬?€+ìyÕ®4FGL J2324.6+3115?ÂÈ[Óu(+À<^ê–À:r®8(eÀ;÷|Gy;U@=eP@¿R%fÁÖ?Л™ðË/?ÒSû)×iß?ýu©dè·å@	Ñq§"=?íïMËdíÀ¿ãƒ!ˆZ¿êªó^1
¿¿îBÜ¢¨6¿ð?ïÿ~‹¡3UNASNone?ïÿK[ìR%?#GïE¸)?"'u»kÅ?#GïE¸E?ïÕ7f8Ãñ?'ƒM?r?udLãžt?'ƒM?r?î{;•6Í?š"ߔа,?¨LF¯<"3?š"ߔа,?ïÃÚØ>¨×?qS>…³
?~"à«"x?qS>…³4FGL J2326.5+8555c¿×n'×%(@7Q¨½#žÀ:²š'^À<1¸£J"@Ä5Õyï…@Vü9¡â?Ìu‹‡ÞY?—½"]?Ǥô^@LÓ±Ã\?n'§¯S¿éTký@¿é'^ÿê±d¿è›ÿ/p0¿ïÿ^Ê¾?ïõl=ÀÕÉUNASNone ?ïüÁ"æB?CJÌØi½h?9óØÏ]ð3?CJÌØi½a?ïæŠ@J+€?'k'~ù7?iu¿µÔ€?'k'~ù7?ïÀø§<ʋ?~‹3p ?ƒ¬aš¹ÿ?~‹3p ?ïò±Q?'R?Pìþí£G?Z]±[ª?Pìþí£O4FGL J2326.9-4130¿âê'¶-ÀPàñ€
À:h8:Ùð¢À<À>-b@D³'>0'@A–EQBé?Áy}Yò吿™hüe85s?ÒӌDÐ@¹fM¼ÌO¿êƒ
€òç¿ãz–~ÜÿË¿éI‰¶Í‡¿åç¼r¶¿ëÈorŒ¿ïÿûbâMhUNASNone3FGL J2327.2-4130?ïþð4êá?1Ã&ƒuÌÞ?.`ü±QõL?1Ã&ƒuÌä?ïûŸJõ+`?``ÒbÜT	?A'Ô+Rñ?``ÒbÜT?ïÊDéáo?}ÈM>)Ü?z݋xÈø?}ÈM>)Ù?ïú\å¸[?;UF¼Ð?FŒhõ'ª?;UF¼ß4FGL J2328.0-2557?î	"±ïtÀQÕ_þmXÉÀ;V"tnÀ<撐Ü\@+È%Eá?þQ¶á¨üä?Û¾ó'ªi?ÐSX!+¯?õF‡nêÍ@v>Ôüò¿íº¸˜baõ?ïŒ<"Í¿åCá9Ñ]¿ÃžÅR…¿éñk}&œL¿ïøVž`3UNASNone?ïøNù©Sü?P?ó.3º?NÄZ°?P?ó.3»?ïö¸éûÝÅ?nÕ¨\1^?RŽ,Dv%?nÕ¨\1a?ï 1.Û?'.ºüNî?›ùÚ=¤Ÿ??'.ºüNî?ïìŠ>>N?Y[`ðN?cuÁ~Á±Ù?Y[`ðO4FGL J2328.2-4422¿ä‹UïÐÀP€^"ð•À;£Ÿ}ß(ðÀ<ôy2?@ mnžÄ%ß?ü4 ½¨?×?(ßÈ'!?ÃCºió¹¡?ä{PÙ6h?üZËE8Ch?ìH‹¿¼C¿î:a?µøu¿Ïßü?Eö¿ÊrÜ@ˆ0¿æršA4Rÿ֓V¿)vUNASNone?ïü˜ÓY?<鞵Êä?;9gÝ3úm?<鞵Ë?ïøZ™É€?d¸Œw›W¢?N•™ˆÙÿ–?d¸Œw›W¡?ïÚ©•KZ?yÅWirîâ?rö+5ZSO?yÅWirîÞ?ïç´T
¤º?W‹úÊgÔ?hK«ò[F?W‹úÊgÕ4FGL J2330.5-2445¿ÒW ±‰ÀQì<âž4À;,|CG}À<}€úfc@a.ŒZkÜ@™HUÚ'(?ÜA?Õ6ڇ rÒ?óšÞ¨—c^@I¤
æÈ?ïúy¾\òt¿ä '+"Ø¿éÖ]Ú¦ª#¿æñhÞë0¿ïÿ%¯¼ñ?ã'+ìíÕUNASNone?ïâUäø‹?xûFË
?mªñu;?xûFË?ïÐòùf
^?ŠZUÎ=û?w†ƒLúÑ??ŠZUÎ=û?î$Íñ·ª(?šÃÿŸv·z?­³ ä…]…?šÃÿŸv·z?ïÍ?°"?m­¹\31?y~à'¹6?m­¹\334FGL J2331.6+4430?À‰Ó¦
äÀ0Q ÄeÀ;]ŒÁDŽÀ<À I·@ í;ÃO |?ý|s%³?ÑìoíÏ?¸N
áÀB?ê–>€nOi@Œ.'ã³?퐜ýç!¿í=äÒ}ö¿ÆÜ@WV¿Ù¿Ðºíý¿Ôÿ¶Äw¾¨¿å/uK¸UNASNone?ïþ»ÇÛÀ¸?'öM
.?$C'CôjÊ?'öM
@?ïþ2Rì 
?LÆ1Ìò‹?,ÚÑ=ÿTÕ?LÆ1Ìò˜?ïõÁßÚ9?bˆ!"ªë??T|@Kãn?bˆ!"ªë:?ïðÎ÷ºZ?J¿$ÁºüO?^bæ‹L?J¿$ÁºüP4FGL J2336.2-0715¿âgéܬ²ÀO§'`4PÀ;Š†‹ŸÛÓÀ<Ë+M‹¤@L}Dú0?ù>³†ªª?ßV·à†=?æƒ4õ«@àÎ&i U@þÎ4Uó¿îWS~WHç¿îùXG"©?êïàªÐ#¿ß2Š@ṿïÿÿ)@k*?î¸"†<ŃUNASNone?ïü±¾Š-?Ešî">?:wj®˜"?Ešî"-?ïüóÓFrž?W½ë!ùŠ?8aeÌk?W½ë!ùˆ?îœ43÷å?˜¶d²ŽÖ?¦>|¼Àª?˜¶d²ŽÖ?ïö–Oû5Z?P)$ûh?RÓ`	•Mf?P)$ûh4FGL J2336.9-8427¿î­˜‰i8À@.0Â?«À:ú..çtÀ<'äö=ö@Ձšt_ù@GÂÀð ?ÅsŸÊ`5ö¿ŒìMñz&?Çf™	Ñ»@~+±Ì?ïÎ5Lèæß¿áV8ñ¹`¿â´1?¾¿ækœ 1£¼¿ÖI¯áÚ{¿á,$€èȬUNASNone3FGL J2337.2-8425?ï÷çR¶q?H ôâC2/?P1ÇZ"Q?H ôâC2$?ïý`!Ÿ(]?VvT À?4þó½\?VvT À#?ïÔ·6?wã\!¨À?uþ}$zdÃ?wã\!¨¿?ïê+ª®7ã?T˜î"N|?eÔUQȘ?T˜î"N|4FGL J2337.7-2903¿ï˜çó÷YiÀRiIùHUÚÀ;S·K[H%À<Ìzü ¯@Xs3©P?úØ»'øme?ÚÔ"Zï?ßwç˜*-Ñ?ú­êk|?öY<tz{F?ïK;½›Vˆ¿ì$2å/š¿ÓzcôF8¿Úƒw
S¿í×Þ
fðÐ?ݹÕcÊ)ÚUNASNone?ïàȐ–ú?qî~èñ܅?o7oiþ?qî~èñ܇?ïmíú#‡á?¤5'ž3— ?'B@»Ï?¤5'ž3—?îê̐#¤?ŸC7åÉp?¯áS6ýÅÉ?ŸC7åÉo?îc>mbqã?œqÍL^Ô?©Ì)ØáË?œqÍL^Ó4FGL J2338.1+0411¿ìúÄûJŒ=ÀK©~+VÀ;LÓî)>À<}3+¦w@!Ž:´w?ü/[7^;?Å1'Y4?"Ó= ¿4«?ÀÚA?Šb@§ákv¿ïÿÿ)@k*?ïì¿B ?î¾}=B¿ÖyV@!-¿ãi¬}Ãû¿ê!ۇz³%UNASNone?ïÿ'†ñLÜ?w2g¾ÛÐ?^C¬Èð!?w2g¾Û¼?ïþnäÔd?PáÓâI?.Ù²¹®'?PáÓâK?ïê1×û??oâÖX/"ð?eÎ(îÀP?oâÖX/"ü?ïùJíÍ?E/îAæê?JÔHËû'É?E/îAæê4FGL J2339.4+3008¿ÔºL[¥>÷À>2É.4À:Ô®ôt±ƒÀ<Œt¬zFî@ Å#
F*?ÿ=GþœS?ËW+ lÇ?¨Ó7Â[|?à?3¡íûñ@°Ø–¯"h?ïڍ¯ãˆ¿ê¯À¢r¿âd2å/š!¿ÊU½â#K4¿ëb¿è¸¼?£o—ß҅kUNASNone?ïý8aD=å?4'
3D h?6<õÞÔü?4'
3D o?ïü|ë˜4¥?[r9è峎?<£>Zט?[r9è峎?ïÂ;Ÿbpú?'2?%J&N?~â0Nǂ¡?'2?%J&N?ïߣÔ	S%?[ŠDŒ¸T?p.ûVmÇ?[ŠDŒ¸Y4FGL J2342.4-4739?Ê?º\oðÖÀP[Æ?À:¤;ðqÄÀ<´;4‰tˆ@žÿãO›?þŸS‹˜O?Í)ß!Ž?Öû" áa"@Öt_Mmq?ýÃwÌ?^:?ç"ÕåzB¼?ß®3Äþw?¿â§'A°¿àáA=â䑿ïÿþR€ÖT¿®O×®¨˜UNASNone?ù	eZ™î?ÀnVh˚N?뽦©Y…?ÀnVh˚N?â²Në|þ?Ö9áµYq†?ڛb)À?Ö9áµYq†?Âm`O§?ªiÀòäFŸ?ëd¹'ì??ªiÀòäF ?à©[*!?½~ô9ºvÿ?ßÞ­I«Í¿?½~ô9ºvÿ4FGL J2343.0-4756¿ÚBäoÅ{ÀPR§Å¬À;b¸N†ËÀ=¥O°A@ ´ió
Ô)?üÇà"9¶?Óã=ñ?]ðv@>†TBw@²&|–~‡¿Ô×ûØð?Öß?–¿do³Âض¿ÃÑe¸Á}
¿é_9ìŠØ6¿ïÿü9¡â=UNASNone3FGL J2343.0-4748?íÃçêÑ0?°wJ•ûä ?±çØÀ©vw?°wJ•ûä?ìHùh—×?ÊrÔ#gå?¿å¸4»AD?ÊrÔ#gå?ëz%N`¬?®ðë¾ñÔ?ÂjÆ}R?®ðë¾ñÖ?år¦ŠM?¼úåáž?Õ²ëdã?¼úåáž4FGL J2346.2-4322? Ö%ŽíŒ ÀQDÜ3rTÀ:ÝW4šÀ<§JNØ«'@ýG#Õó@	q"Úí÷À?ü]ò#žjº¿¤¹OÂ`Z?ؖ;`~Dÿ@…ê⣿Ò`£üž÷¿ížo÷ß ¿âqáÄ«–¿î©;,ü¸M¿ïùL`RP?Ë,b^™éKUNASNone?ïüÝ"·v?†	%'³?9ïDPd?†	%'³?ïÈ}ïÓ!?– ß´-ßC?{Áo}?– ß´-ßC?îÐzÅ+ÁV?ž(âƒ1?¢øS­Cê¨?ž(âƒ0?ïõ–[IÇ?Z™Ÿºb~?TÓßIlq?Z™Ÿºb{4FGL J2347.0-5720?ÕOJ©þ³ÀLÚðZpŽÞÀ;‹¥·µÀ<ã?«çy÷@ö¨M'ƒK?ý ìt2?Úy¤)ëa?Úøäl-P@ y¢ƒM'@<!Gxd–¿ïü£ŸVòÖ?ïÿD¹mtx¿Þ¥¿'6{'¿ãkŠýõcÅ¿ïÿöût€?î÷ôÎs•úUNASNone?ïöÕôp¦L?S#¤;ž$¦?RT³gË?S#¤;ž$©?ïñµZ_?vÔ1Mi?\•ÇKAî¢?vÔ1Mh?íÃúå"s?Ÿ€—Œ™?±à/(Öìd?Ÿ€—Œ˜?ïØ!†Ãn–?kN1Wu¨b?sï<žHµ?kN1Wu¨e4FGL J2347.9-5106?¿(å–`!ÀO–/­lµ5À9£OÄcq¿À<j1ßv½@s€Êë¡@¢%ߍ™±?±X¯ïqgv?¦î2ß6—þ?òDÊÕ{Ç÷@"_õ3d¿ÞÉë¼&6v¿ä&Ë4*ª¿æ`C¢?Ý¿çzȞü·¿çQ	<¿£ï¿ïþ SUNASNone3FGL J2348.4-5100?ïÿ]/OM\?°™°NÌ?ZT»?°™°NËì?ïþdk<ô¼?Fâãy´ê?)¹L0´0ã?Fâãy´ì?ïë:WR´?c%K}²®?dŨ­KN?c%K}²œ?ïÿ¦7¨¢?›Þ•S?Ë9
ë̈́?›Þ•4FGL J2350.5-3930?ä†]-´ÀR.bÀ;XLpñÚ£À<Ç$'&µv@ö‰QLù®?þºƒ-?ÚԎ!ÁEÛ?ár×Ã Ô @҉T§ø?êIWÚ(ø>¿ïHðŽ?ï`?àÓ¿ÍBjCk¿èé£Ò؈¿ïÿs+(x?ÕG$ARۚUNASNone?ï\F'œ)?¾¾í¬9­?"|7/¬zÕ?¾¾í¬9­?ëCÑm÷/X?ÌJžÀxñ?ÂðºH#B ?ÌJžÀxñ?ì¿DGˆ–?¥FR\!±í?¿ÝûW?¥FR\!±î?á
Šlɞç?ÀÇæ…ÍÚï?Ýäë&lÂ1?ÀÇæ…ÍÚï4FGL J2351.4-2818?æú*"3jÀS+à`þG™À;&ˆ|:äÀ<¸¾ aŸW@XŠv;³@ä®ZZ?ÏÆ_u;@?¼§0ž-}?êŽSz
ˆ?÷àO"'é?îa.¹Pï¿æúf=v®¿ã.^œîc¿äîV,\¿â«={
¸¿ïÿþøþ"UNASNone?ïüüë`!?: â¢ö7?8¤þ÷ÒH?: â¢ö'?肋ÞîVÁ?˜c€hÚ¶?†›DjP
?˜c€hÚ¶?Ÿ[#í?ˆ¤âU3Ý?ŒT˜)7¼?ˆ¤âU3Ü?ïw|
°l?ÏÛRd5z?'ð~Iòy?ÏÛRd5x4FGL J2353.2+3135¿ÓjŽ°»À=ªV¼¥7]À:Tð=ëÀ<JHêT@u1æ,@Ø'sâP?·ûø‰iÔ¿§¿6a;a?ív+57ð1@	WS\¬ÿ?ît=¿~0¿ç2–À¡E`¿è~=½Ð°‡¿ÞV`x»þ¿ïÿþBe«+?ïÿì´É ÈUNASNone?ïþÏpÓN?"]Âí­o'?#ò˵&?"]Âí­oo?ïü[+˜]ˆ?bRÆöx?=&£=º¯?bRÆöz?ïä~EP–?qÈÒ>¯­ô?kâº¯jU?qÈÒ>¯­õ?ï÷Ù7ñ?Ô?CL÷ûm?PM€Wš?CL÷ûm4FGL J2355.2-5247?äPS(>ÇÀO#ãŸw),À;žUÀüµÀ<ÁÐ%Fáf@‡Ü¥Aî@[ˆ^Þ²¨?ɕµ‰dBJ?à…°ÿì·@,`RP/@
.'uÏ?í#P!U*¿ÆbK#¿Í¶¿à¹*ù¨Íê¿éþqTÖñê¿î[ÛÞb¡`¿ïý󀕼•UNASNone3FGL J2354.8-5245?ëóÊzS¾T?½×¹'ºè?À0Ö±­?½×¹'ºé?íŽ?½Œ¾y?År½v?³Žš9?År½v?ÞÙSæTS?º|{,íº?à"~ÖÕÖ?º|{,íº?ìÄnF"?£bõòüb?¹ÜÎëZ?£bõòüb4FGL J2355.5-6614¿êD\Þ¨›ÙÀHøSX"À:]RtA}À<Zºà;>š@·Â«ášº@†÷ µí?¿¹? §??ÑO9c£éT@Ñ ;tJU@"é3_ÓÐ?˧9ÓtÝ¿Ýë®ÄùäFfގ–¿ê–—Péý_¿ï‰nÿBž¿ïò
"þ2UNASNone3FGL J2354.4-6612?ìíƒé ò?·E×üã-g?¸"à¶øo?·E×üã-g?ï‹äŇuT?¤‹¦¶'0?Ξ"«(?¤‹¦¶'0?èUu0¸3?±L~Ø-öž?Ϊ+=ó3?±L~Ø-öž?î‰墧Þ?'äF,ÚõÉ?§n'¥Õ'?'äF,ÚõÉ4FGL J2357.8+6839?Ѐ²Y³u@/çáüúÀ:{·0ƒVÀ;'²´ҟ@EóH6¦@
äÏ©?Çw¹…_?·oóegä?ñØ·lwÒ?ÿ$SÚÁ'?ìÙ]ÔÇm¿à²Åº‰Ô*¿é…¡êöÙ¿åá';"¿ê8'üÕ©¿ïÿèž:UNASNone?ì΢?–†?±ÒôòbòÚ?¹ŠîKˍ?±ÒôòbòÚ?ì
HfUN?Æ'ˆµ¬E?¿­¼ÍW-"?Æ'ˆµ¬E?ìFiø%+?§2ñ©ÓI?½Ì°>×Ξ?§2ñ©ÓI?êG^ø"†x?¥în™æÿF?Æâ"íæ!?¥în™æÿF4FGL J2359.3+1444¿ämó»2ÀG ÌݓÄnÀ:ÌhfçÀ<tlâ˜@êx»}š@MvûßßÏ?ÖÒ~ýáí›?ւ[Ü®l@` Ùÿ»7@rX¹TŸê?áhÝ{µƒ¿â9
wt¬¿ãØîª_å¿ì$4'®ÃÍ¿ïèè¡¿'â¿ïûÕctCŸUNASNone?ïë<ßðŽÂ?n·"R‹Ú?dà q=Ò?n·"R‹Õ?ïë¡Yy??|ˆ¶"+?d^¦û†Àá?|ˆ¶")?î ÇX¦-?˜HCaw
?¥óŠu.9?˜HCaw?ïx:" -ø?|ç6÷n«?ø­kúA?|ç6÷n«4FGL J0429.0-0006?ï‰<"€|À?BÝHE0À;*šÞ=8À<!-••@j/Úc8_@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ÒûÏ×g?îuU9y¿é‡V +à¿ãý…Â!M-¿î0£kªs¿ïþx«ãH9¿ïÍ®5öAGNbcuTXS 0426-002?ïÿ'¿HÃ??"'t(òs?ç˜ú?"'t(òrú?ï÷çw2"y?'¤ŠN_Ÿ?P1šÙ-?'¤ŠN_ ?îcn¢$ÒR?š6&Pä
Ð?©ÉݲÚê?š6&Pä
Ï?ïêÏÙu#?Wºx èr?e0&Šïܜ?Wºx èq4FGL J0534.5+2201i¿æD&v|cÀ <Ž%ÈÀ5ì"ÓiŸÀ;˜=)HÏ@"k±»¤[j?ü?ȔhqH?´zá?òõ†@íT¬ª˜?˯¤Gó_¿°^WàL퀿Ð9–m•/¿ÈÙ
¸OgF¿Þ:—Àü_¿Åa2àRÂOTHERPWN3FGL J0534.5+2201iCrab Nebula?ïÿ
®ä¸‡?slD§æ?J#hïŽ?slD§åä?ï:€p±?¿_ðHT?G?˜¯üüQéé?¿_ðHT?G?íõž÷\²ñ?¢êЬ8 v?°SEh{?¢êЬ8 v?ïq€ž'³u?¢@7×îÿ7?'Ïì/©'N?¢@7×îÿ64FGL J0850.4-2558?ÙܝUÌ÷P@&Å«ŸU›=À;CHdàÀ<Qpنïs@û&s\æ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ùwy‰-ç¿â'¡Ã3Æ׿ìªÒ ɤ#¿æÖ¡aä÷f¿Ö؉™qV¿ìŒ$ÁUuR¿ïӜ_F·tUNASNone?í§²'þ?°Ä0EÖ3?²ÇÊkè‹?°Ä0EÖ3?æÍp ?ÒâZÝzI?ÒeÃûÏÂ?ÒâZÝzI?éڎæ[Ë?°NN®pµ?ȕÄf"¤Ô?°NN®pµ?é¯óASqd?²¯Ï |§´?É@2ú²:q?²¯Ï |§³4FGL J1039.7-1540¿³0TzüVš@BKl6KìÀ;/æw˜¾À<Zíl…@[öëYTÛ@θ`?ÓÀ–?"aï?Ån¿³è-?ñéÿ¸‡p@Âë'D"X?íãC ¼
7¿ì'lá)Ñ
¿ãÇ=áâއ¿ïŃAéYu¿ïù™ê!qj?î"Nü½UAGNfsrqPKS B1036-154?ïÿel{?Çu—ô<"?Rn·ª?Çu—ô<£?ïᗜ£VÉ?'Ø ±WÊ?nhc\©6×?'Ø ±WÊ?ïhWj:è(?Œd"x8<?'õ¸¢û?Œd"x8??ïÞdí!,?d˜{®WÞ¶?p͉ozj	?d˜{®WÞ¶4FGL J1202.9-5717?ÝÍt
•e@ևà3±ÞÀ:å¼dŸ¼ÉÀ;É>adžæ@W=Œ¨ou@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ZRúMäd¿çëe>H:?ﳫ=°å'¿ØÎªžœ¿æébßôñ¿ïÿã_¶Hý?á±À6UNASNone?êx̘œH?Å¥ÂhÿÃ?Æü͝Žá?Å¥ÂhÿÃ?æµd~~•´?Ó*ZåÏ,?ҕ7ԙ?Ó*ZåÏ,?㹨ÇB¨?µÉØ>ÉaÛ?،®q{ö²?µÉØ>ÉaÚ?ꢕr¢.?³ŸxnK?Åuª7ÝwJ?³ŸxnK4FGL J1209.9-5923¿æŒÀW?ú8@o¬)ÜrÀ:rrÓ\3À;<¤'D`'@k$†r'@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ø¹µ‹g§¯¿ï,,À/[?ïõ0~Mù¿ãj–â/4¡¿îÓ¬àsGË¿ïù'm-*¿éê•ÀF+³UNASNone?ír½ìÃÆ?¾Û'HP?·,j™áÕ?¾Û'HQ?Ê8^™dÿ?Ð
Îõ¼¶ð?éqèY¦ÛÁ?Ð
Îõ¼¶ð?ދ|ý‡Óå?¶$cvµAˆ?àºA<?¶$cvµAˆ?Ñð¯mLÜX?¼32'å?ç¨IY'Ó?¼32'å4FGL J1320.5-6256c¿±åg'2r9¿Ð¥é^'þwÀ:Ĺ­À:ÃM~8D@!XÒTÌ
/@…Áÿ¿=m?Ù6>`7ù?ÑìD`Eÿ­@=جÔà?æ€á;ïÿªÛ
}2?ïôßÀÅWŽ¿ÛàY¥"¿âr·bWc¿ìp	è·UNASNone1FGL J1320.6-6258c ?Ü i®Œé'?λݡö#?á¯Ë(¹‹m?λݡö#?ïL
Eã~?¾kz|<ÖÀ?œ6~·CN?¾kz|<ÖÁ?áˆßÍ?ºù;M»?Üî@eõËÙ?ºù;M»?î¡'ÍcX?Èt;n-?¥íƒ)Ê~Ó?Èt;n,4FGL J1622.8-4454¿Ö9=u£½@
ß_ü¿ÙŸÀ:?íë*…æÀ;I6_7ü@³›õ>…ø@uuf͔?ÔÉ@v¬s?Ð~®?þ'U_­å?þìrtf¯7¿îîoÜV?ïþê‹út¦¿ë§žªz'm¿ÞJû܄е¿îñƒ€R ·?Áƒ-FŠ(
UNASNone?àÖJy ?Ð<Ÿªd?ßÜSk
ÌÁ?Ð<Ÿªd?áíFÑ\?ÕWö]'è©?Ü%r]ÏÁH?ÕWö]'è©?á¢Îÿw/?¸†Üªi›‹?Ü»Îb¢?¸†Üªi›Š?è_7Óڙø?¶ç\q3:$?΃ °•˜#?¶ç\q3:$4FGL J1758.3-1920¿îpÐ#]A@Àó°fÀ:³!*3À:Ì&€IR@!
²˜@LÌ?ß ?ÝF"µ…'?È5*ÀY22?úâÿýPÎ?þ3³P¤Þ¿íß/ûÆ?ïäÈÁû7™¿æ>Ê€Â2¿æû]U¹¿è?tŸ&ú¿ïÿæ4|ßOUNASNone?×Lj»ÐÌ?ϖ A?äYÊ¢s—š?ϖ A?ÃҘhkïy?ËÚQ[U?ëYåå!?ËÚQ[T?ßL]òé!?¹"Ýӎ39?àtYÑ‹p?¹"Ýӎ39?ÌUÚ>DM?Àˆ|tçé?èø*‰pní?Àˆ|tçé4FGL J1838.0-0516¿~³¹ì¥y?áöѝìåqÀ8͘¢ù"¬À9ïœp
¯@%¶Ê×Õ@3€*?ùCO`Š7?ÖÞEvX³@"Jà£ï3@K¹•ãV§¿èîVŸÉß]?î8†ß'±÷¿ãý+-«4¿êÌ W"ý¿ïÿšŸ¨ý:¿Û
! á÷×UNASNone?à!OGl"?Ú¡obÀhÝ?ß½aq&×Í?Ú¡obÀhÞ?°Zû	_§Ñ?ÀûïÔÂõ?íô žÔ?ÀûïÔÂô?Æ«†ªª?¯?ï3YJ?êUU}9?¯?ï3YI?¶cÑ÷¬F?¹,x¦wc?í3…Á
~˜?¹,x¦we4FGL J1841.3-4442?â3mƒn½À1R`õäÀ;R`îWaÀ<{y¾Óæ@½›yÙ@¯¹À*§ô?Ï;˜@—ä}?­"@ fäÒ?ßrl@gpŸ@
Nܱò+?ê…cíbt?ï^JZƒÚ¿àiPüqÖ¿æÆÙmÄÿy¿æ˜y¾²Ø°¿ÅÁÂ<1µUNASNone?ïåç¡ô?g/fÍúN(?j^àüã?g/fÍúN.?ïïώõ?|b)‡ï?`0q€
é8?|b)‡î?÷…S€?ˆx[9ìð?ŒØ«ð?ˆx[9ìð?ï³ØÕqÃ?qæÄ#õ¸¤?ƒ	Ê #3?qæÄ#õ¸£4FGL J2048.4-2517?Ðq˄xJ?ÀBa$FEÀ;ž6a»Ü»À<Œ~å¹,Ý@rEêE@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?üŒ ŒÒáº?ÌWµž‡êð¿î·Þ"ž­Ö?ÁB‡dð¿êj˜Yþy¿Ðæa=²"¿ïÿÁKJ‹UNASNone?ï4rø!ˆ‹?ž¶L¡ÄP¸?™q ûÎî?ž¶L¡ÄP¸?ïp›C×·a?¦Ï/¸š?'ì—…	Í?¦Ï/¸š?ëqs)=Ü'?¬qãK»–?Â:3[g?¬qãK»˜?îÌ/s?¡"J,;2A?®?}xÛ?¡"J,;2@4FGL J2106.9+2455¿ëþíFûùÀ-Ýãø¶À:êﲪâ—À<3¯Rhƒ@À0"eÛ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@	Ýä$g?ïÿÿÊPË¿â=zŸXub¿ê•ñ¤ª[¿é¡­>¼ÿ$¿ïü¤–LÝÿ?¶Ýßnºó±AGNbcu3FGL J2106.1+2505MG3 J210642+2501?ïþ©zoöb?2k›f"~\?%hY™ÍV?2k›f"~2?ïàkÜy?˜ú¨¢YC²?oð"ç#‡?˜ú¨¢YC²?Ä`Q¤?•¯1#_/X?¥#¹úåË?•¯1#_/X?ïßbAõ8Á?aÓàÊ&?pNßcŸÇ?aÓàÊ&4FGL J2325.9+6206c?ïþ4ê "h?ëê*«¥4ØÀ9¼iVïSÀ:øqž¨Í@5ü+46=@¡ÿ›¬?՞ë@]ñ«?ÁœßÉw?öæó^ÜÚ6@xýz>µr?ç}ÈMKŽ?îq!ôœu¿ìz_í{n¿å÷QÕR¿ïö¸ÞÙ>Ë¿ïürAeûÝAGNbcuNVSS J232543+6208290?ë¤Üµt_?ÂkÂÄHål?Ál¥*.?ÂkÂÄHål?á!´çoíþ?Öd~qôu‡?ݼ–1 $?Öd~qôu‡?æošr1?´Ç=mQ'©?Ó Ëé˞?´Ç=mQ'©?âW¹"؇?¾‡"z?ÛPôöNó?¾‡"z

==> SOM_VIZIER/4FGL-DR2_prob_catalog_3classes <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  595 / width of table in bytes                        NAXIS2  =                 5788 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   72 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\4FGL-DR2_prob_catal...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'cos(GLON)'          / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Pivot_Energy)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'LP_Index'           / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'Unc_LP_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'LP_beta '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'LP_SigCurv'         / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'ln(Variability_Index)' / label for column 11                         TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR12    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'HR23    '           / label for column 13                            TFORM13 = 'D       '           / format for column 13                           TTYPE14 = 'HR34    '           / label for column 14                            TFORM14 = 'D       '           / format for column 14                           TTYPE15 = 'HR45    '           / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'HR56    '           / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'HR67    '           / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'Category_4FGL'      / label for column 18                            TFORM18 = '5A      '           / format for column 18                           TTYPE19 = 'CLASS_4FGL'         / label for column 19                            TFORM19 = '5A      '           / format for column 19                           TTYPE20 = 'ASSOC_FGL'          / label for column 20                            TFORM20 = '18A     '           / format for column 20                           TTYPE21 = 'ASSOC1  '           / label for column 21                            TFORM21 = '28A     '           / format for column 21                           TTYPE22 = 'Flags_4FGL'         / label for column 22                            TFORM22 = 'I       '           / format for column 22                           TTYPE23 = 'AGN_BDT '           / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'AGN_BDT_STD'        / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_BDT '           / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'PSR_BDT_STD'        / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'OTHER_BDT'          / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'OTHER_BDT_STD'      / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'AGN_NN  '           / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_NN_STD'         / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'PSR_NN  '           / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_NN_STD'         / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'OTHER_NN'           / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'OTHER_NN_STD'       / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_RF  '           / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'AGN_RF_STD'         / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_RF  '           / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'PSR_RF_STD'         / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'OTHER_RF'           / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'OTHER_RF_STD'       / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'AGN_LR  '           / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'AGN_LR_STD'         / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'PSR_LR  '           / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'PSR_LR_STD'         / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'OTHER_LR'           / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'OTHER_LR_STD'       / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'AGN_BDT_O'          / label for column 47                            TFORM47 = 'D       '           / format for column 47                           TTYPE48 = 'AGN_BDT_STD_O'      / label for column 48                            TFORM48 = 'D       '           / format for column 48                           TTYPE49 = 'PSR_BDT_O'          / label for column 49                            TFORM49 = 'D       '           / format for column 49                           TTYPE50 = 'PSR_BDT_STD_O'      / label for column 50                            TFORM50 = 'D       '           / format for column 50                           TTYPE51 = 'OTHER_BDT_O'        / label for column 51                            TFORM51 = 'D       '           / format for column 51                           TTYPE52 = 'OTHER_BDT_STD_O'    / label for column 52                            TFORM52 = 'D       '           / format for column 52                           TTYPE53 = 'AGN_NN_O'           / label for column 53                            TFORM53 = 'D       '           / format for column 53                           TTYPE54 = 'AGN_NN_STD_O'       / label for column 54                            TFORM54 = 'D       '           / format for column 54                           TTYPE55 = 'PSR_NN_O'           / label for column 55                            TFORM55 = 'D       '           / format for column 55                           TTYPE56 = 'PSR_NN_STD_O'       / label for column 56                            TFORM56 = 'D       '           / format for column 56                           TTYPE57 = 'OTHER_NN_O'         / label for column 57                            TFORM57 = 'D       '           / format for column 57                           TTYPE58 = 'OTHER_NN_STD_O'     / label for column 58                            TFORM58 = 'D       '           / format for column 58                           TTYPE59 = 'AGN_RF_O'           / label for column 59                            TFORM59 = 'D       '           / format for column 59                           TTYPE60 = 'AGN_RF_STD_O'       / label for column 60                            TFORM60 = 'D       '           / format for column 60                           TTYPE61 = 'PSR_RF_O'           / label for column 61                            TFORM61 = 'D       '           / format for column 61                           TTYPE62 = 'PSR_RF_STD_O'       / label for column 62                            TFORM62 = 'D       '           / format for column 62                           TTYPE63 = 'OTHER_RF_O'         / label for column 63                            TFORM63 = 'D       '           / format for column 63                           TTYPE64 = 'OTHER_RF_STD_O'     / label for column 64                            TFORM64 = 'D       '           / format for column 64                           TTYPE65 = 'AGN_LR_O'           / label for column 65                            TFORM65 = 'D       '           / format for column 65                           TTYPE66 = 'AGN_LR_STD_O'       / label for column 66                            TFORM66 = 'D       '           / format for column 66                           TTYPE67 = 'PSR_LR_O'           / label for column 67                            TFORM67 = 'D       '           / format for column 67                           TTYPE68 = 'PSR_LR_STD_O'       / label for column 68                            TFORM68 = 'D       '           / format for column 68                           TTYPE69 = 'OTHER_LR_O'         / label for column 69                            TFORM69 = 'D       '           / format for column 69                           TTYPE70 = 'OTHER_LR_STD_O'     / label for column 70                            TFORM70 = 'D       '           / format for column 70                           TTYPE71 = 'Missing_Values_Flag' / label for column 71                           TFORM71 = 'I       '           / format for column 71                           TTYPE72 = 'Category_Prob'      / label for column 72                            TFORM72 = '5A      '           / format for column 72                           DATE-HDU= '2022-01-29T22:24:43' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             4FGL J0001.2+4741?ÙùË WìÚÀ,­º<§À;J,Rƒ[À<‡éÐ2@Qì̜{K@Þ¥šXÜ:?Ë·¢C6`¿Q¬gsùï?µz'Ÿ'h3@ù-@*¡¿ë8罓ô¿?讵¬ß¿á"c+YJ¿èÙE¡Iç*¿Ú!*•»¿Þ
\¿žúAGNbcuB3 2358+474?ïâ•á/
?nSòñlD?6:ÐVBá?gÇ=DBÊâ?j£¤âzD?bfâP¯Rc?ïßGëڍ?ƒŽ'VN"?0w'š?"œ?EÓañY'?nìÇÿ‰"·?'kåΝԴ?ï]4¿áh!?‡I˜ƒÜþ?Yå_£#:(?^Ž~€â?'»ýOR?†˜÷.ˆ?ïÑ°ƒbm?S<"&±NP?6ªâÀ»6?!šþi-€±?vy´5¢?S8n\-@>?ï¹-è׬?z"'¸gt2?;Ÿ…Âöx#?1o[¸‹%?€âxOø?z+\$C+N? Ø<Â?"HÿÛêb?GN)ŠÅú~?_$Ë·ß	ý?‡$U6ø–}?'TíöB?î×'±AMu?'}F°F6ú?dbíB0¤ª?gôàÏÿ€U?¡GV`do?'Ûâ8?ïtäõHÓ?tæ›°;?K/+¬d'"?A£ø©²³÷?‰èκ¢?t‹i+šéøAGN4FGL J0001.2-0747?ÞÕGqÐõÀPӅH©¼ýÀ9j8³¥´ZÀ<‡þ[@ŠÝÓÛ3î@"<½öp4?°Fc熝?¨ø\óvè?úƙ¬äÐ@ý"õ[?ïïXÌý¿á®?Ffí¿ã¤ÊOD
ò¿Úþ-b8Ú<¿èa~J2Կވ–<"AGNbll3FGL J0001.2-0748PMN J0001-0746?ïòþÎbï?J+;
©ç?%óËùìÆ?dâJ~p?WCôsY?H šL8µ?ïçkÌK?p+kzä®?6¬'8o²f?Gü¡'iš?e¾·IN›Î?k»I.׊¿?ï¿qi¬ð?fû›"ˆ?TLæjøÎ?TO|ÌM°Á?{4óÿü?b†¯<ß%Š?ï­ÿ.kD¿?]©ñM1ü?\ý|ñ®á?@4í''€?€ýôª9äx?Z_)–´Zc?ïæSx÷Ž?\ûÞ¿ßÅ ?9b<Jz¹?*(0uUr?f€@CE[Ë?[$²
*…£?ï°8¤X±¿?†xáf'ƒ?KmÍìº?]¡y™=c?':ú•Ÿ?"àMã+Â?Ë_(H?vMß-åÒë?`vC=–]U?b¶:2¯–b?…¿üVhœ–?ræéþ"Ⱥ?ï;—Š¥ú?xçí`ÕPª?qpüƒÔú?[HV<kûÛ?"F²y¶æŒ?u{§gßuAGN4FGL J0001.5+2113?åyèÂÍÀDužèóÀ8^Äþ¢2À;Þ¿Â"O@O
"M@bœº¶IÔ?¡î[3?ÄRÆ6ɾ@L¦CÌ«@k˛ŸXJ¿Ï® yÈ¿äeßBp<ÿ¿èÀFA,ðú¿ìoN6ĸ+¿ïÿûÎBÓ?lÏÉëN¡AGNfsrq3FGL J0001.4+2120TXS 2358+209?ï§ú*±	?™Hv%#?€ëÅ®ÈòL?'¾Þ‡SU?dV¾ÕG­"?ƒjàÓÒÀü?ïØpeSýê?qKñ'ÎR?@žáÙÆÐ?J¾gÂgúš?q³ñS¨ÀF?p*ÞÌcÑM?íI
ZD?¦<¡é@Ã6?¢jü-zœ?øŠlŠTÉ?©Ó/x¤¾?¡µqR²è;?ïúޫК?0¶b…P8Ï?(nw¢ç?˜U_Tlz?<ӕqºÈy?)ʍFr²"?ïiûzùà?šð»Á>?«C´6ˆ:?™ˆŒRŸF?gWv ¨?j°o_Æ?ï–TYSÕ?ŠÅ?Vòï?KA?n"¹mnøA?‡Œ‹¨»º?‡"åT‹0?ìËOá·?«´R3|Ð?¢¤"x¼V?™ûŽÚzˆ?°S76Å[a?§­ýuSl£?ïïð36ì¯?RÑV,.£?CzåjVW?='oúƒ4Ö?Vb&v›lŸ?NçېxªAGN4FGL J0001.6-4156?Ö$L^!†ÀRÓÃa@À:DOÀ1³×À<]yÞon@ —ÀÍe#?ú®oês¦Á?»xö"¼C?±ÛsÖôï?÷®·`,'@A=©-á:?í½¥|üªá¿ä«Kb©îQ¿ÑIò&ùi
¿ÑíñÀL5ä¿Ü}#Â'w¿Ïb9°ûµîAGNbcu3FGL J0002.2-41522MASS J00013275-4155252?ï~BÜm?·gWK¹E?7µHŽþTž?&;R·`K?±ÒĊ=n?·iQ]ð¿ÿ?ïÜÈÌü·:?r·Œ³´?:Ex¤ù?EüÅZÈ¡?oî";M?pÕl—!¬
?ï~ºnŒ‹Ð?}§Â½"yZ?Xâ·DxH?VZ¨
C°?5
qæHà?|ùïV¤ÑU?ïc©#¿»?jû›	#Ÿ?M×G*ùyª?1ÏAŒ)¡4?'œ!Gô…?jx0î/¬?ï›÷r<ÞX?®ÈYt¶Ab?J†¡J{‡M?;`Ç]–f?‡Y¹[‹)?®Ì²Lx;–?ïŸÀñæüh?‡Ð¸]·½²?P€¬b==?]r	{_Œú?†
3_Ìðé?…ý*|o+ ?ïÔ̆½?Œ¼DÇã·~?a¶Ó®×T?Ri+ÿ–…^?‹øµø?Œ/ŠÝ@ú?ît«#7p7?…ãexQ`Ë?`R<•Ë?M5¤ç%u?§°*"Ž?…£ëW&'vAGN4FGL J0002.1-6728¿ãm5/EÀH{Râûã;À:'J7[·À<™øn;Fþ@ m#"'ÿ#?úؒ2>?Â	ˆ–.?Äõ¤îŒ@\	›Š4¢@Ï$'ҁî¿îèÌ!¬"2?Ï ¤Ð¯Z¿ÕºÀ°´¾¿ÔšÀ[¥B¿ÜÄ°ž˜Ý¿å«`"gAGNbcu3FGL J0002.0-6722SUMSS J000215-672653?ïçõ¡q5?RÂ?ޚÞ?E"P^^¹?7O9·ìºE?bÂyÕㅤ?Pg¬ÞW%6?ïÇ¡ÉW¼?vNC½äæ?J¨Wjk^?QÖÙJÉz?xÚb'Û5?s›ý"u$*?ïâä¹?o9;ˆ(?]8¨·"<?IÌ»
F<=?ˆxòVµs‰?mÁ¼¯½'5?ïCJØôÖà?l¶l1b–?cÀrE*?Fýå@ö?•£î¬ýl?jþ[LnMÿ?ïÎÏï"×?e;3Ēëy?^Aéåýlr?S'‡
¥'M?qŽ
ý<?`=ÿÿyÿ=?ïQIËÈb?•Žv–Xs>?]À몡ì\?k» ^푷?"Èôzì?"£Ú…à
Î?ï1œjâՀ?ªò˜œ?nvù´¬?lÛ`a]HÌ?•ý¯"Äu?~˜¡¡û¾?î&T‡Ûp?‰a¼0èî%?t®âKM'?bóhT«?«
úFúÞ?ˆx(Êh]AGN4FGL J0002.3-0815?Þ:Æ$'§ÀPöK	éÎÀ;\tì;'À<¥S"'Û@ 'ev§Q=?þÚ ø2¬?Ñçq"Á?Ã7S=êœA?óM¹Nè›@ŽM¡sÙ¿ïÿú Âî'?ïþ–ÞÔ6N¿ÝüK€ª¿Úmïÿ
z<?ïú;/€÷AGNbcuWISEA J000236.06-081532.4?ïÚ©[zò\?n~£Ë«ø\?^]Ñæhßz?`TÝYçB?f'»½Ô4?dç¿£¸¼(?ïğng37?|.;Ø~?R°'–™G?]Ii$¹¢=?y$zÒ9ä?vâIi%?îÃ=°h?•6Ùçڞ?"¾GÚÒL}?ˆÃ
ít;?9&
ò??1§á¾ö?ï]Y™=B?uU̾F»"?c!çc­u®?Ož=£Ù
Ò?'ððYŒ?t7¤®ãê3?ï¶"T¤Ù$?|€.â_;ë?r­üš JÓ?r)_ôaç?r@ÙDw;?t`K*†øh?ïo	˜ã™Ë?'ñÀ倽?`X•=J€…?j'U_‡iá?º@.ù{?Ï£:i?îzôÒx*?"û–ŸûC¿?'†dOŒ7?"ÿãñÀó?£¯%ý'¤?';6`/Û?î4±œ‰|Û?'XzH#7ñ?uN™+纼?k?ƒÊ¹šë?ª	|?' ڐæ´ÙAGN4FGL J0002.4-5156?ìéSЮûùÀOÄþ'Q~xÀ;Á!\qÀ=dmgâg@ ÖKã*\?õ˜/6Np¦?áióïP…T?ä†Íyšö'?ÿuäô
ÿ8@/tæ±ÐG?êK7 ¦ê¿íƒgþìÛ¿èšð{þ~ ?ތ¦ æ{¿áL#ßÙ¿ïüò™åï´AGNbcuWISE J000229.20-515227.4?ïàxJ`î¥?s‡_É?C%[ïŒ,þ?AÕáYÂ?j¾^çÃP~?q¨ØMq?ïÊÁ.UuJ?€Ÿ½ñ?S	\2 ‡·?fðOêÁ,ð?uÝÊ(?wA^[¬Œ?î'PZi
¹?šK°¨_ø<?m0ŽA¼'ç?pôÌ	tC,?¦ñsǹB?™õB•Yvœ?﨔Íñ©À?næˆøœi?D-á¿Bh?@Íȉ¦€ó?"—ú†dÊ?n44é,?ï«£1ý?Œ;®Û4?UææهS?YX‡Öx ?'Z[]H ?‹Nƒûà|%?ï†a1"?"X/;ãÎ?[ŽØÂnº÷?s-bJ?‹ª7•{?­s9®Y?í$E6¸›?¥Î+õÕ ?pχOߣ)?x;Åû
Ƃ?µÐßoÖkv?¥˜AÁö—è?ïYíº·?‹wü"ì7M?R¨
5 %?YúT
Ù?œs"#o#?‹1
Ä,ÍæAGN4FGL J0003.1-5248?¾3M8±¼ÀOdüó0À:R"O…yQÀ<x|àü.º@ xŽÎ9‰d?üöYSXm?½°''¾?¬îþ%	yÑ?ó_6Ç<j?úжç2T¿éß5…
Ó¿ ©e>ž g¿áìáàZHK¿ÛY¶T»C¿ÑFÆbûLè¿äXY]ig£AGNbcu3FGL J0003.2-5246RBS 0006?ïºF†]bî?p; 3œ{?@úP³'û?1V\ô*xý?€^¹Y·†1?o4Õ{CV?ïÆ嬛º?zC†~"³?Q)DκXn?Y	œ¨ëè?xBØ»0é?uõ—>q?ïaŽæ7W?{[šêÙP‰?c
JÃb?P×·'£
:?'lyý|U?y£Îò°ýß?î¹NïU?}Üõ´J?qKjö~5?YZ+\¦Ã?¢A±¹ìl?|ŠÁŠZ~ª?ïX/†_‰?…qšòÁj?W¥X'«?J¾ôò×Ê?"É£rlv?"Æþ,¥?ïS8ÇFÐõ?—€ Èñ?d'AÜîÖÖ?m|)Vøú?"žÓøâ–?•ƒVD÷&?îË$B¯?ŽANŒ§"?nGñÆY?fš§¹ªt ?¡k¬Êk!?Œà";ª€?ìÀW¾$_Ó?˜^ñÿ–‹Ž?ƒØkøí)?tôšˆå;ã?·'A_Ý"?—Ú™±Dð›AGN4FGL J0003.2+2207¿«mä›0Ù£ÀC°½ãû½{À;0')ˆ†À<w2>@­o@iBªI•?è¢Ç
,¸?árh!ýU×?ïýt³è@1¬šþ¨?úMEââ¿ä;ËB^n¿í5K Â€¿èuˆb—7?Ð;œ£º.å¿ïfKÄ#°ß¿ïþ'"oAGNbll2MASX J00032450+2204559?íÔBRñû—?®Ä©¯Á|?y¡JPý¼¸?^¦>›®¶?¯‡±Šˆ ú?®$a¹Lu?î<'ÕæY™?³µƒr^?–d‡ËJÈ?­÷]¬ôäE?¡Ž¿ˆÝ?Ÿ¤ºùªj?ìg–¡¹ðô?¦†kÛG?™SçïϏ?';Q®¬!ó?¶nP÷ô€¶?£YÂ<p¶±?çˆÿÇ1=¡?¸7£Ä
žy?kx
A'?"-TH—ùz?ÏΠT§TÌ?¸Bí¦NB_?쎈Ä_@?¸¾Ží—hT?†ÂŒ9Ü0?Šêñ¢…€§?¼³:23Œ}?¸pïDȑ<?ëqþ?Wü?Ä°UdL?©²jâ?ºþ"H£?·ÀYqÂW?¶Áä­Oj2?êåý2¾?­¡±ýÿÏÍ?šo÷M?'¹/—»?ÁÜ{~?«)OÑò?ãºËà`ñ?Ãjƛ8â?‡óúš,À?š¤d%ì1?מ(žsŒÙ?Ãí¯r–AîAGN4FGL J0003.3-1928¿æؾ&Z¡{ÀS%.ßç[ÄÀ:‰HºƒôíÀ<w˜¢ù"¬@qŒž3‡@w°év?À½mÈ°?ϊ' U`@
D žq@œåGB	?ï¬ýw޿δ]?KDw¿â‡ôiÉÈ¿ä`‹[uN¿ë°SO2m;¿ïÿùJYQAGNbcuPKS 0000-197?ï®dQŽ=?zË^±í?r†pIw˜í?sSµƒŠÝ?vGgÅñÛ?iDG0Ú6?ïÑØM<&?uùTOm'‰?J¾ôy´¤?Uô«÷n§?s»úÍÕ .?r-jÄápD?îÉÈY†À4?—pÉÝ'd¨?'{x?ƒ'ê?'"$£‰˜¬?•K|ˆÅ>—?Œeªð'F ?ïž?Úã!?cÇ8
ºŠ?ZßÉÕÿ¬ð?B7Þ¿àÿ?…?Í×V?a¸%þ›Á²?ï)¦wM"]?'ef#Yþ!?‰¢‹Ÿt¾³?‡!ñT\á?‹ó։¶ö?ƒÉ~5Ï?ïŠéÝ¡'Ð?2ÀDžæ?]<|}3°?jQþ0Bg?‰ùˆ?‹ž8õ^?í¥H,ó?¢·Ë?£Lm:òÃw?›`u¿'{M?¢cŽ>Îp1?•}áWHfK?ïNF4Þ?~¹š'&V?p)ú¡…š?^ف¤üí[?›‹¸–›¹?{ùÏ@òÇßAGN4FGL J0003.3-5905?ïåòhâ+ÀL{¢£Y6À;Cü¯¨À<¼…Ñe¸Á@Ê\ñ*$@L€S?Á\¶î¿¿§~Š°¯?åýºËø<?øŸ5dæ´?ïíŠè%èMþraF¿åÉ3¿Â¿à8G¤Ú?|¿êwMt'I¿ïé\ AGNbcuPMN J0003-5905?ï¶@?£ºœÍÅ_	?W±'GoU?€ïÇ<+â¬?~ó$ùc±?Ÿ!Œ¬F%›?ï¢GŸj­¸?€… ¬ðþÎ?aÃî¥7N?cÆuÈPá?'ý|¶ª?z¤¼'ãâ?ï%ë¾÷Äj?‰-ØPD®3?w{ú{Ìt?{ÆUÚ8?•|©¨Ï³?":…Õä?ïGåw=¤%?r!¨üN?~'Ð8A?b@æ·\¶?Žò¹áÜ«?mS.<´ªW?ï{Ԋu(?"›\×mü?bœiä:sº?[>jB'?Œ˜0p²°ò?ƒ"¿qßF?ï
½Ñ1`u?›Šµõª¾?qEp€ÓE~?xj´&×;?šVéÁ†9ï?˜7Œ¡H—?î»_5´[¬?'—Y%õ­Î?€ØUJ֞?°Î:rY? ÷cç?œ?õáÝܲ?íÝìëâLø?õûŒn\?–Ôàǟt!?'Š
EÉôç?¦¶ÀÜS¨t?‹ÝßÎð,AGN4FGL J0003.9-1149¿ï,Ä­»³ÀQÄÎp:ûÀ:ՇΕú©À<¦[·¶»@³9Õs?þéÀùYó'?ÄNmRé²?Ñ[!¤?ã@
¾á77¥?÷çÔåõé?êªI¥Ò?ïЊA7õ¿Øarv?!~¿ãMDVq%Ý¿ãªèvv~â¿ïÿò"²¢AGNbll3FGL J0003.8-1151PMN J0004-1148?ï.f«ì¿?—CûâQè?€mOq&è³?~¥´êáG?—C‹x¢0Ë?'ƒ	|ƒó»?ëã<ÙX?ÇùõŠ\e?°'ŒÎ	W?¸¯·™›a?³fXÝ8k?¿P.ú»?íþÛ:×?£¬ÈöS"?¦gþÝdKc?›ñ7fþϚ?¨ÈEÃî'?™Ä08Zy?ê²òÀH*?ŸŠ¤NÍo>?¯u6ð¤dÆ?•Ï'ª/f?º­Î‰)MÆ?—·o¼})?îRÎ	?¤rëêP>§?"ìvoÏÄï?S°CMq?¥)o¨
ó? \†'¼k?êd*D)Ù?Ç'ü;>?µqlÔQ–ð?À:azÄAc?·naÙû
Ç?¼·RQ±xˆ?ëÑB™ÇU®?§µËu×?°–y'ì+?¡R՝¨]?°ßq Cfc?Ù­*?åt°ÿ;ßÕ?°Ë]ÈnG?¼G¦ÙY^Q?¨rž_ÕgK?Ì	h˜‰"?«¹4¸›ãAGN4FGL J0004.0+0840¿ï€ž¤#ÀJ2ìž#lÀ:ߍè‹o4À<&Žà4@aÖQZæ€?ú­Yº†y+?Òè‹o4kB?Þ×e,)ª@,œü$©-@oô0¿äõj¿'{¿ë÷]>Êk?«§½ý.È¿Ùý¥ýÖ.¿í¥è\uKÜ¿ä
NÒËêOAGNbll3FGL J0004.2+0843SDSS J000359.23+084138.1?ï>NÎ^?‰X"ý¹ºÝ?w´ÁiŸ‡l?pJeìÓYW?'R¥Äi3È?"þwþ?ïŒüt¨?•ÁùS `?yX·`°Ã"?xç0øÆ4?–‡ ‹´Ö@?'xl¾¾Bü?î6ÏFÇ1?˜Ò(±ng?""UAÍ?‹¿€qã?¢Ñë¢1
?'½a:{¨¢?í–1ìGx?«Oµ¨w?'i1¥'ˆ?jVƤT^­?µV(:7²"?±I}fKþ?îEe±ûÀ?ÅΌݡñ?pCރ?†ãK[¡{
?£q¤Ëæm¿?™9¡/'?íãÐñŽfú?¨çà8Ê?‡_¾]?ŽZæúw4R?«ë0»Õ?¥¼}T›þ?ì¨}©'ÏÀ?¤¾³'ă? ‰)óŸ¡?•ãw'6¢??²w~%¾²?Ÿ¹ÙJ̑o?é'Ç×ðld?¥¡'øŸ?Œ«òÝc»?']¬…Çú?ɖ!pyK?¤ÐݐËAGN4FGL J0004.3+4614?ÆÏkì`LÀ/µ¶¡è´À:A´¶U'À<	*K-%@Hó{bKú@7<'W…ù?ÄRéF€?±:Ë^¸?ìt1ËT&É@m­3Tk<?é"€­ºc?Ò,&äñ0Ú¿æÓu}°"î¿æ6J²È¿ïÿÿ²}@¿ë
CQƜAGNfsrqMG4 J000421+4615?ïòñí¡6O?KžÿՖ‡?4Kô'~û?&m',`Ž­?U	'Àg$"?H?$Wï<ž?ïå[u¶TT?mOÏõ@÷Q?8"™Lòõ§?C ã-7B?g'÷‰Ñ?jT-³PQ¸?ïsäK͝?†.xÛ«YW?kªR?pƒ?ŒC±qè?"dOà½ð?ïµÊ'4öW?\å³|n?`•Uèû
?BçORAoE?|ÐÑ.ƒ9?XØ÷§½°ç?ïæ‹]ÒÕ6?\2àüÔWS?GL—»œ¾ª?:bvCBs?c¡|ã۔?XŸwëþ"&?ïºKrð˜?…O…]Ô?K…$ß^Òû?[¨ÅmÊ>@?i¡ææo³?ƒ¼"É
Øo?ï%´gr¢?†"9½?t•IþNÓ?xúwX½¸ˆ?–"Vò"Ò?™Ou'?ï@!ùØ|6?wHùYÏÕm?ujä@ô?a2ÊÃã8,?'¡K´A7?sê²{ëÆQAGN4FGL J0004.4-4737¿ís?oNÀPâk΅3±À9酿ÈŒÀ<ê$Ìh@G:ï•#¾@o-d½û?´Á«†?·»Il°'@-  ôØ@½Î°|µ¿Öš¢bë݉¿äà}ƒ¹^¿æwž™¿ã%ªê#õ©¿éˆÒ!Š_¿ïÿàU?ÍuAGNfsrq3FGL J0004.7-4740PKS 0002-478?ïóC$~Ò?I0Ê·ã?07B…Ó°Ü? d[³~A?UkæÄùÑ^?FÏË-«L&?ïð©gå8÷?dšäñ${¦?(ÔÔÇË%/?<™ÐCúS·?['•ÜZ:\?bG맍Ï?ニ'ÎÍ?k?Àa
õ?V;ýk¬õ?VþY)?{-·&ª<?fáØÉ't?ï÷¡zl5f?4a㚥¥o?$´ÿ¼.?ôB%?Ly©ñ»;?2ÿTjMçc?ïâ4å(Ò÷?_ÊBãHû?CŽŽ:Ð?5Š_åUP?i	– Kªš?\p⍠´b?ïÑ`"FKò?€Ñ¥Û‰?<O=˜p«°?TgÂí?uŠÂ†åÇL?~îAj¸Z?ïˆ8e¬é?yV¥æEz!?d¶lÙ],?d΂¬¬÷?ˆÄ]<œ›?u`[7Ù?ïè£3$?Uk&ÿÈ"?=‡Æ¶?/G¿N?c»ûŒ/{&?S—ÊЈðAGN4FGL J0005.9+3824?﵆`ƃ À7¸dàÀ9œSÆP±ÉÀ<"Çȁ@p!G£X@j˜û(¸?¶Ã0òZ¦?ÈNÇ"é¹í@ô±î$5i@
LPóãg¿Ë&'¢È¿ânyZ^ñ'¿ê
ªB^Ia¿ëD§>ȽŸ¿êg <¶j¿ïÿüÉï£AGNfsrq3FGL J0006.4+3825S4 0003+38?ïåˆfÛ1?'‹*3»ßa?]ìmµe×
?uX³jd¢?WÅu§?pCT÷Ô¼s?者ái<?˜…ï*D?a0†iWZ?f"Ɛ
á?'Ä©:?|!aœýs?ï3iaB?JäÇî«??yù'´[.?}}¹H!?"{õ{?Š×9ÅðûÛ?ïhÁg
r—?j/cÊÄF?|Cpfö&^?]†£'väP?‡­îa?aè$˜Åò?ïÛÔn¤ó?iߪ`knœ?eumyȯ?`ВO‡?]lHùO)?YdŒòM¡?îÁ5¡Äد?¢¡6ä1°?…l̅Iîp?–¬|¥aÑ?"åƒ$ë?˜$«tÒ?î¤4\un9?—¬(DzL<?‡^B°ž?‡z×î	?Ÿ¸¬Ày¢?"10oK¡Æ?îj'J9?‡Ø5$"Ìë?"ð:=¨'?|›ÿ]—W™?ž½•¢>-ã?¯š0q"´AGN4FGL J0006.3-0620?êe¢@ÝîÀP¨òù‡@À;/#Dže/À<­\Ï
ï­@·-¶œ‰¹@ØTÛ#§¥?Í"ÆÔeH?ųNáåbÆ?õOl@!ð!慿ç0Ýî]@M¿·?ï.K—Ù¿ä'§
öbȿݶßz¤`ó¿è:Ë­èÛ÷¿É~-W|AGNbllPKS 0003-066?ïðKôít¯?Pbn[ô?8?/æíogw?Y,'®¢;?KºLF ‹?ïÝR4;'?oÑÿžQ«l?=(ÀÕÓö?ET7†Ö?o
FŽ&˜I?l<H>'Ü?杻w)Ï?t$"f·»?XéÜ#Ã-Ü?ar½éÛRƒ?ƒ¦¦lðª?qŜäËß?ïÇõgÿ e?Xѵj‰¤m?D6ÌU½¦†?)úÛ]¤ÿ?y~rmÐþä?Wú7G·x?ïÛ\›rè?b÷󢿪?MÆΙH@'?FŒýøs?m1°¦w_Ê?`DnŸ½ñx?ï nԍÐ'?‡–Ï®·5?Pãø¼»;?a´Áµ6ï?…ÇËÜñ?…I醀ˆ?ïmZÙ6ßÝ?îåJ?aÍþ§mž:?fXñ²W$-?å
eœ'?{m¿ûÊèy?ïWmƒLai?wSõ#ÆÂ;?X·{ߣÚ?F
ÃÙìÔ?"ÔN¯?w€Êm@AGN4FGL J0006.4+0135?ïôEÁ͌³ÀM¦&þq‹À;'Æf>À<¨Ð©*0@t×#x€?ûÚЛŽf`?ÕaÂÍÅp?ԍŸ½~ü?ü
9‰Ž‰›?ý[ÛU{²~?é&>ÚH¶?Ž"Ñ,û-*¿Õ¹¼å#/Û¿ÝOõ`¿³_¿å¶³ «Ü'¿ïëñUBQ´AGNbll3FGL J0006.2+0135NVSS J000626+013611?﷞uT—?'þÌr‡g?RùÕ ßÅ·?YÁäØÜv?rP[?€Z¼œÐq!?ï¡&=¬]ì?ƒ=1Y`?béܑ?gÒÌìYf?'ú‰"oí×?~›ž»ô5½?îøZ»sš=?'Ÿˆ ÉÄ?QS§Ãc"?ƒt¸t½Ú?˜Kþ¾ÞãÖ?‹ì¶×Uˆ?îŽÈ8?"†Š"2B?ƒ%,ûÈO?fTsLÄ?©fD…$žn?€_ƒ×'%?ïšUèG…?€FØa.d?^ý¯XIJ?Y¸üú©·D?…žtš'°?|懪¢	9?ï
ëzO@?š£Î]uÆ?uªÅŽÞ‹V?ž='–l™?™7ìÆ?•´ø`G•?îy´Îm$µ?–É=~Ä3Õ?"7¹|k;?…î3ØRD¤?£VŬ)V?"`›v=žò?ìJAA¾¼?˜Úå¥qû+?‰‡ŽquͲ?xð/>è6J?¼Œ¼&'j?˜qàÊ­#AGN4FGL J0007.7+4008?å]×Hs-ÁÀ5ùÙUmÀ:Ë
Tí˜À<fߥ¥@"Dˆ›¡?ÿ¿Å}M3?Ãß4®]uý?ÆøĤ•@á*¢jùs@	ýÛV}e1?ï6è)I¥e¿Ý'‡"-D¿ãœzõi¤	¿ØëÚcä+
¿êWAï8²¿æÞ+	Ë[AGNbcu3FGL J0007.9+4006NVSS J000741+400830?ïæ&œHÃ?ZÀW\';?O‹Ÿñ¾âU?EÔ)¸
z?a÷\²R4?SÄlI]û¶?ïÒ¿gkþ?us,úŠLV?L	@tÊZ?W]¯QŸ{?sV¨uS?qoš'ð@?ï‡F<>8?ƒ
nº<…?r‡öÂá.ã?z¨Þ`<
Ÿ?"êuaâ?z~õ?ïk«Œá$s?e˜îGÉ?sO:Ý?Qmôƌ?‹m":ᦙ?bx:8?ïÎèVÁ?jÈäóM¬¿?c†,ZI;?[;«¯ 1?nqëUÕÔ?a†Iµk]?ïzÔP5Û?‹ZV·Ïf?`¾ÅƒÈn?lòK¯Ô`?:—KMÁ?‡ÿ¬»7ã—?ï@¿°&?†QhRyÊ??>¨¿?³õÓ?"hbåaö?Š¯©4óûÛ?î–÷'¥X·?€YsN'JB?…voŒÄÓ?k4ÑÂÏ£º?¡2ëõèí?{ø÷Y/Ÿ•AGN4FGL J0008.0+4711¿ãQgÜ]8•À..¥.ùÀ8¹¢‰à¿À;§=áâއ@ÞTû½?þÛ«©gm?¦%"¤DÃS?´A﹋Ò\@®jv–_R?ýÉ
mAL¿ßÚ£}ɿך/ ~û‰¿àŒ
ÑyÛ¿ÛsËßgD¿ãéoÐrs»¿æ3R3ÐèAGNbll3FGL J0008.0+4713MG4 J000800+4712?ì÷SœñN?²WNÎø©¨?‰wìnÕU?ª4Cà@?µeŒR²u?ª†–¦3g?ëìåk ¬À?ÀbItL?²
èŠo?¹_œ3,J?­«;"»?­¼"ñ/ ?çûãúw>?±è–Ÿź?§j"pÛkh?›ÏÌ¡«?Ê5Ë9µên?°0áÃè{?èHd6¥s?¡]˜¼˜ÚÔ?¯e(¦Kà|?‰mL¶F`}?Ç$ü}ƒR? ç ù	kº?꽜qÿæ?ºº¥ÿi¾F?•F‡,¡Í?–Þ¼5]9?ÅFýÀ_¬?¹N…{ØÓ?æ˜ÔNîœù?Ê;Óë¤ÿ(?ÆŘrt‰?Çe!ŠòÀZ?½®,£¢%?¹tÓ¬›ò?ç>Á›¸¥?°ÿâ
è	–?¥`
`)¥/?—£
ëó+ý?ͬö8!Ž?°Rˆš
0D?âÄLÁ†?±ïPê—?ºìiRÝ{#? 
Q·b?Ó¼MyÁž,?±í{ÓfîAGN4FGL J0008.0-3937¿ïžÈ6SèÏÀR¥UGZ1¥À:½ÆßîÀ<xLuúX @Ñ"³U@+ã	O4?ͺš›!Y?Ú
‹t<è¿@»íx:¤@7Š:?îãË\4¿á롃rç¿éï¦`ÒRÉ¿ë:Ÿc2)¿î_ÌqæÍ¿ïý
':"AGNbcuPMN J0008-3945?ï3N¿‰Jõ?u-QÍ?z3æòð?uÑñM'cK?"›}C‹?‰<'ÈÑ¿?î|úîâæ?±0ž}ÍîÝ?"+Q¥T±à?¡›_MŠ¥Ê?5P€[Ë?¥	U£§bÑ?î!÷¦a {?š¸¦[£é?"d˜tÅ=¦?‹É¿&FÚ?¤.9cÎÜr?"\¿2UHÏ?íE¶n¢±,?'ùHhí?¸"\%Ž¾?€XåU
W?¬È‡ë1Áã?Œs¹Ö½öÍ?în''#0\?œ¢Ø8?Š»'/¸?ƒ|¾†z»?¢hð¨;?—…\–q?ì2að
?À+ä%?©ñ³æ:ËÈ?·Èi0ˆC?±v*üo?²ÅúèÂ`]?컡q²ÓZ?£îy_RÊ? ÜJ>º)?•ôŒ¶/?±´ÏR­?žÊÞæ?ç³Þt"Y?­ùiyp?µÌ™ª+OI? "®NR5'?ÆJ9V…?<?ª8\­sùÉAGN4FGL J0008.4-2339?ïÿÿàSÀSì6ŸÏ=ÀÀ:Èeü´%À<{¼Ñ­^@!"þäÌó¹?õ•ôäC?Ñm>Fâ"?ÑͅC÷%¼@xCx%@påÆBð¿ïîÎô©‹?ïùÑb]Ã*¿ÆJ>¨nڿǯ³ ÿ)¿¢/¿œsÏ¿éÍáõ¨äAGNbll3FGL J0008.6-2340RBS 0016?ïß+|¹?—"g5X?TŠ4i®"?dÄ`ßY?Œöî¡mTk?•ì:êüQ?ïÞ
•¦@?sŸ%bxº¹?>¯]97ÍU?Jü¢bÄ%A?n~ˆ=ž?q‡.l"Œ?íå¨|q¦È?ŸÖú`qÝ?™8i¶¤ƒ?',«l›Wá?©¿*!ç†b?š"'éêD ?ïC^
î?wû¯'µÄ?G҉<i_?7À'oéo?–Õ©5)ç?wµ…M©K~?ïiòWÔZé?š™' îG}?_Ø.2?gÿ]ŽÀ"?Ä2"z?˜ô(^e]?ï«Sù¯âd?ˆP]¯kd"?N]ožÕ·è?\s|–¬ê?ƒE*¤<äy?†ŠÞYÀz?í›>ŠTW?£ÒÜè@=?‹/óXiÝñ?ŽëøϳS?´5'¡?¡ÌTWèm?îlÍÃ9G—?ägüœ%ï?Pz_ÅHB?Fòñ\Í®?¨¯PÐ}?Âñp‰ïœAGN4FGL J0008.4+1455?ã¤Rò/ ÄÀGVžšÀ:J‹¤äPwÀ<fjbti^@¡Úõr?ÿÈ+}\L?ÃÖÅIُ?Ä|í'hr°@_&¼,k™@Ðÿ¿EÑ?ïñÁä;~[?ÀV5VNb¿ÛAÅݚOw¿àðž'ú¿ât"Ì¿ïÿÿ)@k*AGNbcu3FGL J0008.3+1456NVSS J000825+145635?ï¥b]]??tRa@¬ä?a|éՅ|?S#ëï18£?'HfÎ!ªÚ?qéôž¢•à?ïkIF!«?ˆ±b¸?mEBÚuí?l1G}ôt?Ük˜'×Ü?"ŠTχ‰™?ï9ƄÍô?"¹p6?scÕ^äu?pƒ¤›Šf?"1ÛÛS?€òF`6ùs?îåz…?œÍÎ¥û?ª_ö›ä^?kð,>÷ˆt?¦ÇŽéž?z¤GZx»?ïYè
¸76?‡ñ\V˜?x¼xàGC-?qp~;eû?'ÀñôºØ?áÉ^-\Ú?îN1ï;a«?¦Eڛ:°4?€ü²²/j?"£Kúu®?¦Ý´` Ov?¤'©÷pö?îœgíO#T?'¶÷Ú^ß?'—N‹âJ…?Õñô°?¡"­"M¦(?eË w»@?ëÇ+&@Ô?–´ˆ!:ý?žUŽÈrY–?ƒT…c?º1ºôCo}?"‡P
UöNAGN4FGL J0009.1+0628¿æ+xïÞÀKo$cŒ—SÀ9ö™"º]À<HßݵR@(É°7À·@*¢jùs?¶½'é("3?§_¾EdR?ñÇ=áâއ@Œ@ž'?鸞—@¿ÌGNž·Ì¿ãéˆà
ò1¿ß@?
Vñ¿á¨–¾•¿ßç¢ünÐîAGNbll3FGL J0009.1+0630TXS 0006+061?ïÁÌLX?r˹º;õ?J'G7½Æ??úŸÀ0É¥?zîÈqô?p·kî»áú?ïÏÉۚ‰È?q‹¶"Ç\™?Fɔ†`?KcbÁ¥?uJï}&øb?n`ÎÜMq™?ïxL–ËLß?w',I¿O?bÖ/t:?[™¾´±z?7N€(ŸÕ?u§oç%t?ïGÊLÿ¼?l$v¿'?kî{å?L ;ÙrÉ?"ˆõÌ9BÜ?iø¢Æm|û?ï…\&W¾¿?zo;ÀT'L?\1‰£ò?HáƸ¬!?‹"Å&æ×?x܌ȤÃÊ?ïr¯ŸëBY?ŽsÚïڀÛ?`
Lu¢º?tªìD¨?PÄî¥óA?‰èx`5·?îñxÄ·?ˆ¯·]çÌ3?rSÐÛþژ?k[¢e¨?<	±ßªƒ?…S"rUlu?î~"¯œ?‰–°¦¾´?'
,nã8?jŠˆªž?©•Œ°Xþ?‡µ8ªåAGN4FGL J0009.3+5030¿ïÊMùTŒ—À'›oâæê…À8mKrÅzÀ;•L''Ù@»-݈ܳ?þ\Ü_? Ï¯Ù¡ò?¯ãçñkg­@§óþiýË@˜p=Ö?µ,ü€kö¿Ý€Á›ì/>¿ày`^dL¿Üdµ÷ž1¯¿ãL
Ìsá¿á¡ê€¼ÓÛAGNbll3FGL J0009.3+5030NVSS J000922+503028?ïӐHÀ–¼?oÓi×Ý©?:ݼÙÆn?5L9qŸ'?tŠ
"Øh¥?n ë/RñÇ?ïå8î!õã?r·ºÍãü~?4í¤Š8øÅ?DßÄïQŠñ?h)]ZÇÌ[?qARù~³ô?ï•A-¥]P?ƒ‡,!£–+?i€±ÄõD;?tòÔî	U?"Oˆ,K?€w6=4Ü?ï±­€Åüé?aýÚÓJ?KxŸ5?0ù$‰í8?ã(60Ô?`+ÇVҁ?ï³8ûZe
?z1ŸYÖñÎ?@ÔÃ\ak?:?Ï0­?'1cÔ«ˆm?yjø2Šx‹?ï¾­áû?ˆNAuxú~?UJÿ??w{|ö'B^?{'–"SÑ?"T[º¤uÒ?ïs‰W,6À?‹¤­Lh‰7?nʀ/Ú?}ø§ä8á?‹k
?=}?…§ìۚvã?ïTGé´Ë5?z7Ä"ÀZŠ?[¶Q`w¾?G#¸è¦‰?"»¡ªÝë?yCøeŸrAGN4FGL J0009.7-3217?é3ë¿×ÀSå¶ÃvöÀ;
Ë
Tí˜À<ÄFdh_e@I%Â1hX@¸¸]©ÿB?NjÑÅZÄ?Àq<XJï½?÷­_™Ã‹@л¸¨Rš¿ì)ˆ$&Oö?ïþ"4­†¶¿Þ5»8OÒ¦¿ç0ý~E€=¿Ùm"Ãqx¿ïÿ÷Âé±AGNrdg3FGL J0009.6-3211IC 1531?ïÞ®erde?_H7ó}å??u›\ÀØ?1Øþí%<?mbú¥¬ù?\ä­´Py?ïâÉ´r¥?oOíRñ?9\(u‡Šu?FaÆÜ.#?j
ÆlˆVã?kŽ'D²¬Ñ?ïqºûǔ²?|[ç|¼l??eveÔoQ?kB»T•¹?Ž3§–?C£?x3ÌÐó‹õ?ïË`¤HR?Y'"mÑ?M1idé?8Zp½™t?v¯™k…Æ?Wc4àá?ï¹s€¨?wziáýb?UÁtºÌ?OòËAï°?}Öˆ	´Â?u¢8fŽÃ?ïmƒ'?•æXëÒÂ?\<ŠüD	?†Ìñ~?‰0"@›÷?dh¼*]å?ïlúªo?‡ä>]§³µ?o)Ï&¯Dc?pfhp«'?›íE{$݇?…2¨ÒOKJ?ï~'ù<Az?us××,£'?]úûŒ·?RuóUÜXA?Œœ"U­k?te'\Ê!AGN4FGL J0009.8-4317?ßà‡ÉQ\ÀQñíåKIÀ:Ì{¥'Ì À<¿¹!]¹@¤ð'õJ@_¨†œg?¿ŠŠ2‰~?–ÃEÜÐrk?Ù|xl·c@¡d½Cî?ïý7˜ól¿ãGêüó¿àeê«%)¿ãŒÿÂÃ^¿ÊËîÖaöë¿ïünEWøåAGNbllSUMSS J000949-431654?ïÑ5ìdÜg?m¸"_?C…òÖsU?<þ èûŒ¦?tôK{²] ?kTãõÕ?ïãI2ùÒi?m²k݈W?40%Êb>·?@šÆ8â¶J?j0Ȑ,"?jÀã—5'?ï`'¨Ä'?"$ۗ˜ö?Zc‰èЧ6?Qæ積$?'TÒGéA?ƒ¤?Îû5?ïÞv–Æf½?PUÕûõ?2Œ2«šÿÛ?üØÍì¶?o7ãåy¬?OwEPI@I?ï"Ø©œ=…?ƒhÚ`¾n¬?\† Ê,?X»ÐJb©2?‡9y(­@?'%ÅX܇w?ï³Àz½V?ƒ'JÎVûê?E¢çh£T?Y<}¹.)r?¿WW£Ÿ?'s'Å ë?îß{¾Å֗?'ËÑ£kís?b òSCÞ?[O´=‰? æ4îBj?'‰ÜG)?ï¢Ryï/?n
ϑ22?GTñ»mü?:!
ï'?…ûDâæ6?m³@ù¶5AGN4FGL J0009.8+1340?â쀈óÑkÀGüU\Rç.À;W
F9 5À<Ÿ"Ì'úò@5 t-Þ?ÿ1-=¾§?ÝI–a€Îr?Ìô@ÚÖ?ñDœ¸2@ý³Š²K?ïâu@ýA¿ë¢&Á	õø¿â¦2ƒ
¿×Ï`ۍ
¿æÊf¿ïþ^	 '²AGNbcuRX J0009.9+1341?ïA©ÀÙ#?·e´	¾aþ?q²ÁÁ‰ß?–T9F?"^"ÎRÖ?²‡Rpðjý?Á­4?ƒE%>?`QžnB»U?eÌÃÆ‹T?"='ëë0?}ˆxZìÌþ?ïTžF–V2?7‹Ä??gžä%e\?h¸þßÓ?'xZ£P?€¬4Ÿñ'?ï$MÓ%4 ?tÆå.Nç)?[(€–ÚÐ?DP÷–e?™Ã½™#5?tQ1õhEè?ïy¦ëÍÕ? 6›ˆIE?eÝAf3/?oÓle7I?Œô¹…/E?
ôƒMg?ï2ñî^1?"÷®Š²ð?eJ"Ó\|?r‰ðÃà{?—`'yà?'Æm¶\‹?î桞!?Šˆ¡ç«QP?pâpUY?oÂãE.eH?žó0.‰ä?ˆVxô7Ç?í£óùü¹?"E:±Q¨1?emxRpëó?_{}ĺÑ@?²4ônöY˜?"7[™ŽAGN4FGL J0010.6+2043¿îæQ¶´ÀDk&¿‡jÀ:àÛŽ,~À<W÷7Ú@ïùR¼»]@þÜ~ñw§?Ê9R‡w'?µ|Û·Ì5?éðüVþ—@
ZɈ'?ïÌöˆ‡ù^¿à‰Éb4'¥¿æ8a¦
Ec¿äyïøK¿ïý÷è‰ø?ïå Jù"–AGNfsrqTXS 0007+205?ïæO×Ñ6?…Ä0{M?4Ä8"-«æ?0}Jìv"?g èèÁ0?…À7&ؒñ?ïµcN®ä¯?{Ê¡äª1?S'ÕðPwI?X9è£QÝ"?€6џۭ.?w†ÔsËÛá?ï£äõsÆ2?wÒc•sÀ§?`\-YªÃD?dMw‹×j?'ï·Xªd»?u'»üŒ'?(Ç?\Å8Œl+?Dh¼'Ò?)Xt\¼Tõ?|$B@"?[éQdbv?ïØ墏?+?hP
Dה_?D\:þÐÆ??æûÆGÒ?q§\"BO?g¥	IâŅ?ï;§ñÿ"Ô?•5«dpŸ?`,"Kl3?ky™™â-?–…q0©G
?"8ëÔ°ä?ïnÛ4ĂÑ?€_—ìЋ9?c¸Ð!³1…?b
Ôaò'?ZþÏ	…=?LÄn¤aj?ï'Ù5Äe©?bºýÇâq?\À|À|©?JNûÊ­¢?™8Ù3?€ß«×²KAGN4FGL J0010.6-3025¿åba'àÀTÞ?»×²À:-úNwÀ<‹3b-Â@g@õ¼@$
COàé?·Œ~Óð'Š?»)Üâ‹S@R'IðäÚ@Éh>WÔ?é¡ªñA¿âLý|íç¿å9ΛÙæ¿ë÷…¿â¨°"rпïÿ÷fÔJpAGNfsrqPKS 0008-307?ïøòØاT?@Eºje?[S |
Á?'¥–º#?II2}¶ì'?>ÿF¹Vþ?ïîˁÀ\?e÷Ì?2>Ç?*üޅ"-?;Úá¯y¢?_	`òv9?c'Aßè"?ï­J1Hð?xã"|g;Ç?TP|Ý/ÍK?GœX^ú¥?'0ÝËQ<~?xa![,?ïõÝ3™­?8ôŠ´pn?$QAXE? 3"O?0?S@¢ªíu?6õ!¤dW?ïñq°­˜?Q‡4ªæû?$ŒÏ@]
?íÕú1??Z‹~]‰¹?Pâ9¶ÿæ?ïÈH""v?€MÐ([Æ?=³¹'B?P±3«‰tH?z¿º2õÚ?~»¢Ë[?ïOd÷Gìö?‹NTÕM™?b<ƒv#{?X¡ld•Ëk?"ËЯwªÆ?Š›Îoý?ïâLÍ|äÇ?XgÙý?=¨»Òa?/ڛÁ=´‹?jKé¯$?W"Üýà)AGN4FGL J0010.8-2154¿ê'ß9РÀSÙ¡ß¹8›À;3ö Û­:À<»:{&@jˆûf¾%@nLa…V?ÃÍzFÃý¿«H^éop?æGߒ¢."@ž¥]òú^?ï߂ˬç¿Þšù*3°¿æý¾Ý ¿äƒž?ò¿à¥R©®e¿ãûxFbºàAGNbcuPKS 0008-222?ïÚÓ?z
Õ?j6jm¯¢o?Bãkn¯R?8§¢êzۇ?p9òëö'Ü?h‰#"T—?ïÅ7šÔŠº?zÒ̖å?Q°5Ìov²?YØ¥ò$T?xø%9üC?uÎ(¥ç3ï?ïdòPŠ?{1CŸ]#?cg?A+=?Kí%0JÁ?ôÓÓ±€\?zöC‡¡ò?ïÊor¿ ?XÇÕ,Dê?@óDS?(ý¸rÛ?xÅÁSÅ?X4Ý]å͞?ïµîjðþt?u«ÀUú—8?R*²ìàî4?DHìRÔ[?€?é;ë+?t'UàÍ/?ïêú›xR?§M͘m­?VÃ
Šø›?dඋ…@Y?Œ¬ß™šu?Žiü˜Î_Í?î֏ö¥Ô?¬Ë¶³l?rê^]¤e?m³ºÎ»Ãõ? 9´Ç;v?‹@aZh\?ïK?*•Þ?yäi‡(¹?YÙ®=Õs?Kàڙ**´?"ÿý<0{×?yBÅt®E«AGN4FGL J0011.4-4110¿äDٍÇË©ÀRn!ÄuæÀ;D°P$ÜÀ<³@ý R@v^í T^@(z§f?ÐѦü-¸u?ÄCcW`€?ðö›r¸?ù©«?^dº?ç"0ý
'¿ç§0@9«ó¿éPÁ^.´s¿ä¾cþW3n¿ïý
ýn«.?äógkI$AGNbcuPMN J0011-4105?ïÌÊ£I=-?pGüqiʀ?V¿¬*þIß?T \¯–û–?sêÃ3Å?k°$3V?ïz՜‡¾.?'›>2¶M¿?q×Ÿ'éÏ?~wHä…Þ?ˆ'-}¿È?‡Ø2xь ?ï-ŸvŽÞ?ˆ~ñ	³#?uvÇ9<p?sÁ)óœÙæ?"î_gÆB,?…–üæ'ñÛ?ï/t‹\?w8¶©Ä?rº[Þ³?YA)Þ0?•oJjÑ<ñ?t'¹‡sòÙ?ï…ŒrÄ?†u"†Ô'Ü?cË2¶$,?^´To;Í?‰Îº¼þ?"ðÓªF
?wŠÇ?©¯Hç×=Š?…¼Y"°|?•«Ôæ"÷? Vhn2Ëu?¢å.6îÃ?î¤D=¥/­?"3èyvp?€'¸û›Ù›?|Kêí§ÁX?¡—
æ, C?'{{©ø?í=é(¼Ñq?—õ—«´¢?Š´_F E§?{
à݊¾?²º*Ó
9Â?–vžÆ=âEAGN4FGL J0011.4+0057¿Ó?d©ÀN&¾œˆacÀ9ô–Å©ÂÝÀ<N­\Äüõ@L€oüè@IHÜä.?»ÞÿÝp^?¨:g³?êþ;¹ÿk@ö5¦Õí¿Ýù¥ÞÍ«¿å溌¤¿¿å×w¶á¿Û(RšǦ¿ëøV¿ïÿójÆGxAGNfsrq2FGL J0011.3+0054RX J0011.5+0058?ïâ;w-¸?aæU€®DÛ?@üÅÙy ?4wòxóí?i…W'kš?`4"VdŽ?ïð<},ˆ?e«P¼‹*#?*±SԊå=?=Òλì?\0Úþ:Æa?báh1b
¿?ï¶/VÚ­5?xX{úÉ˖?bPñ(†Ü?o$ü	`†ê?{¿Ü#MY?s9.À?ïî•þjºÅ?AWðU2Ïp?-1l<‡À?µ
N?_-ÒܓaÅ?@"ý¨ØÀè?ï¸Ü"Ðh?}È%zU?V/];sŒR?R7ǒ\UÅ?~ÞÁ_éò?y«.2WÀ?ïÊÿýfH?€vmƒ‡Ò¦?;aÀCbd~?M+@R>™†?xÊ#øGAæ?¦ó0þ?ïŽy—	‹3?v#^Q÷?f{nΦT?qÈzIö'Ï?†Â¾‡ãÚH?|°ŠEl‡o?ïÓ°'^?`õ3'Þt?CWšáº:?7 a©·´G?s½Â"c?_¡ZÓ=.AGN4FGL J0011.8-3142¿ê¶—;ùÞÜÀTõƒ¥À;N²™DàÀ<ÓNáåbÆ@ 9ûIaó»?þ²ÜæöC¿?Ì]TS:?±]íÆídÈ?å>lý"O°@…'¤Ø'?Ú%â]ã°¿ëÚúWI'ñ¿â€
¡©2"¿ÔÞ¤»Œ¿Úyb&ñ†¿âd?Ÿþ¶AGNbcuSUMSS J001141-314220?ïòåôÉ®?OÉk¯š?(7ùWÐ?Lª¸W?Xq""Ouà?N	œ!@AÃ?ïÖÔI?s_ELw<?Bhø›a¯è?K-¤,Ga?rHÖ[âl?q0
Ïw}4?ïšw¦¾?s¢™ßúë?M ¨p?6)7I(g?‡§á ï+?sB2 þH?ïФE9¸?WzfK'4?&("ŒB?MgŠ˜?vù\)!
£?WNM*¬,=?ïà]n¬AM?d³h¥kl?/E ÔñC4?";éÀU?m®7|–C?d)Póð͒?ï£Q[gYÖ?ˆB…­öÀ3?JOf€Sˆ?\O~©á‹?…†²·!ê¶?†$ɝtBé?ï3ÅÏØoî?…)'pfŒª?Sç2x+@?G]Ù<ƒQ?˜HÕ>²ÙŒ?"ÔE=×
?ï`z͌Ìh?xÌDš#+?=CäёZÃ?1ÖÉ}
"?"{–¼T
—?x½æ
! EAGN4FGL J0012.0+7043?V+ìÔ@ 9(| À:Q/|À;Á2š†ÿc@
žÇ2@=v?ø="?¾Ñ8Ñ¦Ñ?Š›ÓRt¾?Ïý"ÀÁќ@tâÕø›?ï^0§g¸¿ç
µÂÅ¿ç
ˆ~¿¿ä'1}Ñg¿áEÅÜïüÆ$<kAGNbcu3FGL J0012.4+7040TXS 0008+704?–eÄ?¡j=–¦"•?ba>(ş?WB²¨‰?£H`°³«W?¡Ž¿µ‡î?ëÂ%²þ*Ï?¶00®bmL?l½\:=;"?qÖÚ'n˜?À"sšn×?µ­pŽæë»?íè–~n?›|«Iæ?{ý(Ä¡-'?vªÃfhV?®}d¡ï?™Ii@æn?îÄÄ«ž²f?xFÜRÒ?mˆh=Y?NÀR6© ?¡Û3ðVñ}?w"Ƒïà?ìÆà.~m™?µ0™¹ä?w3FMhû?p['‡bœ?¸UÊ,¡ƒ$?´½Ä¨›R?æ5ën…ç?ÆÖµhy?x¯>wW ?…G²
!ß?Ó1lôõàÂ?ÆsÁڀP?꺙Ä¿É?°H%B5­Ø?RꔦB?…¿Àl8¯Á?à kٙ?®]hi_ê?ìnr~D 
?";²¢mí]?†¶ÿT5@¼?o âðnø9?¹µŒ$¢2?'t	?,9AGN4FGL J0013.1-3955?éf–õÀR»ê šª;À:¼b~À<vA
çI@½PdÇTé?þ¯¼†-¬?¸|)ò?½€{:ˆçñ@æ"FsØ@øv3xR¿îÄ"YFB?ÜR–»B᧿ཨ6ëN˜¿ßɯvz° ¿Ü¢‰'JG¢¿ïáGãÄ`AGNbll3FGL J0013.2-3954PKS 0010-401?ïè9lT´Z?T¤
œç?:€£ïo?,R=«fò?dvt½‰¾?RLV4´üm?ïÃN´Ìƒ"?ƒÆò£C?XOo˜­û?q9|;ýi?xDÉ®_?z§|fñ"?ïE à9?y]'<;7>?gÿ9×HC?lïø®üz?Š 7§ÿ?r~õpo?ïfí ¦!?k	øùÞ?mzi(¾µ:?RJpÏf~;?Žæ´N"P?h)Йma?ïÏX½ÜD?e™h–]?QÍæ
ù°`?E(†h…ˆ?sà'w² ÷?bzV—Ã)?ïKð^ç?¢(ènC/?m±ê'å`d?ŒåÁçö²?'é"Ÿ~¹X?›˜_.z?ï»ð[5?‰ ¸mÏy?xñ¤ÿȇw?zÉ œ5í?˜,·±Ýˆ?"pFësm?:í"?‡QB™«ØÎ?ϟ# "?m6󫌡ì?¡»HlµÍ?"˜Q"ºóAGN4FGL J0013.4+0950?妈vËR=ÀIóƒ@'À‡À:þ¨ø².À<Y·ø)qé@ (ÇÉ@ёW«¹?ÂGÞ;	@q¿±6"K~®‡?ççÛFSË@¼ë-`
'¿æt~7¸~¿éGúÀ{ٿ♅CÛ!¿Õ!â"o¿å®‹cuñ¿È2G%˜âAGNbcu1RXS J001328.4+094942?ïÊ£µ¯ØS?oÄv@z?BQ2"é?3ÿÜù529?xcþÎÅÔð?nš"sí5—?ïÄTQL4?wÊޔW0Û?Iÿ5PBsÃ?R["¾FÉQ?z•ðÁ˜l?tç­ÝÂ?ïO¼Ãa¶?"ÇÌ̑?_!-ÌgßO?a"!G/äÔ?"õŒ±:?ƒ	&­Þ\?ï{–X
qã?ok-8ñ?H,Ȕü/?1þX•›¶*?—bs_?oDÙ?ïjo¤A'?ÇZµÌ?XC"h"~¢?K܀'Eï?ŒœÿÀð²?‰F<Ï3?ïzêp1ýd?‰—óº9?THtcV?]eƒ(õ/Ø?ŽÄÂc–'?‡Ö"
ŽmN?©%|?"*ÇphT?h5u"Úi?g¸Q£]S?¤âN©Ù?'Ž+XF³±?î4ˋ{–?'fᄖ‡~?eT,1t1Ï?Wט#îÜ?«^†B4?'e˜gÔ[AGN4FGL J0013.6+4051¿áËsEòÓrÀ5svæj±À;ªáÀyØÀ<ž&~ïÊ@â¦J,@ÓjZç­#?Àz•ÈSÁ¿ª4
x¹z5?êE&z¾@@Û+'9֐¿ê ÛýÂ8¿Ð_f,"ÃI¿å¯wè]L¿âF(mÝS-¿ëyð¼–ä?ßú1Ÿ_VRAGNagn4C +40.01?ïµ·ÿ­—?vŒ±@Œ²Š?\k,Oe'4?R"hFý Ã?~	4ø~X*?t&!Þ¿A?ïºaFÿæ?zZ#~1£¯?Q$O_ú•?Y7'MQ?~‡èèôb?vº€–ÉG?îŸ1
"F?—õ‡¾ì2š?t՝÷Ñ£?{{CY^Ó?£r?1 	k?—:Nƒ¼O¶?ï˜Ü\aÖ?i2
ÍÆ{?Z)¤–Þ5x?@ÕØ[š?†·"YÓUß?hq#1G¨?ïM°Õ¨ò?ŠÎððí?r}%Šsý?hþ"o°Ðä?'¾À‰aV÷?ˆŠ(†ˆ¥?ï;‹?—›Q·|?`Ûߌ‡€D?jWähUñý?–€ å˜i§?–‹jŠk?í¾¿Éa¼?¡©%´·±?|¾Å¨æ?nßEœÙ?°C©ŽhÀ?¡ÏþÖ@?î'Oëû'0?‰·ý$0öh?tL}nÝ?c%£…u?¤a~ ›?‰Ç'Ú.AGN4FGL J0013.6-0424?䝠ËxJ%ÀPcgM3HÀ:îÍ´SYCÀ<9òYNP@gzÃ?°D@Zþ¾·`T?Ԉx47¿±ÆÆ£gùŽ?ì´Ê(,o@r! 
Ò¿ì?"ÿ%åm¿ãm•ßû¨­¿êÑà2_¿ÛÄBÚÆ	º¿Ù›pß;9g¿ïÿÿÊPËAGNfsrqPKS 0011-046?ï'W1%x?‡±¡ßnY?SÆ{O°°?IqÊ`?ŒñdBV?†ýÔÙ|,?ïÑ«Ø¥6õ?va!Íïu?G4Ô΀?Rëóÿ¤º?tCy&‡~9?s™rÙAŸ?ï"Oºl;×?‹äåó9s?jq$°""?h*ˆÊ²ø?˜gä ?Š¡ß®éÇ`?ïf°Ùôu?qì#°ò–?BZ–ãx_?.n/S¼û?'›9=ª¡?q»Ê»Œré?ï\ÉVƒ?"f£q5ª?h/µ'¤ÿ?`!°í†ËH?™î"Bõg?"r/¼>à?ï˜9i?‰!y)ŠÛ?R'ˆ"òŽ@?bÀEAµý\?‡Ÿt£5¼µ?†úvÍ=•J?î/`ú°yŸ?šà"ÖHëd?w@›fó0?s—Ã&ïý?ª!ÜòÕb,?™dE³«x?îζ?"@T}›8?[j+ݕJ?Q•Mýâ`?­CM:'d?"ם‡ÑAGN4FGL J0013.9-1854?æ
ê‡PtjÀS…âlvKÀ:m» ÒÞ_À<…©²'b@K¶¤l[?ÿH‹¤äPw?¾`»ô?£Yÿ$ãº?æQSåZbL?÷¦è\JX¿¿êÝ´±M†¿Ã ÝE?û¿Ýc-˜pû¿ÝdŸý5ö1¿á—¬ÂkJ¿ÜFàd.RÏAGNbll3FGL J0013.9-1853RBS 0030?ï¼ÓËCµ·?pêz=xþd?C9JM½?4.,JCbÔ?.ù¯Ý<?pžqº>j?ïÄòìØA0?z¦ƒ~y~ƒ?QžÌƒƒ²?WzùDËÉ.?yÖX1‡q?w%Œ;%?ïq|qÀŒ£?)¾MÙ«Æ?dü{•êcê?d.ñٙ]?ŽaęŒ(y?|L	yĜ?ïÔÉ#'«?uþ¡IQØ?pªŸ2?T‡š"Õ?™¤<…×?t?äÈ™?šD9k?}•Ý씜9?WÒ=í{äí?N44@Ãǒ?Šå'½ø¶š?|=<6í?ïR'
Ï».?›[µ§Ol?hIڕå"?vw3êÈs<?'±üc~¯§?™/+É:?ï&ÅFp§³?"f¯üÐR@?ozMßhÿ?ik Ðu!?—8
uyøÁ?'<jrR?íà¢T~1‰?,YcïIÂ?€½'ƒZÄn?oƒG2oš?­ÆzTQÒ?0È÷_…gAGN4FGL J0014.1+1910¿ãÙØ<ÜCÀEiÕ^kÆ"À:¤z
ˆ?À<ƒ€!ùO@ Y:ƒßs@<t$•?ÈùùUÁÓu?ÉD‹ÑYú@—Oµò–@
{I.óŸ¿Í-÷I£4¿ÜÔì@…4¿ãŒ'Á)i¿âñ¡§Úû¿íÇçÀn¹¿ïøðiŠAGNbll2FGL J0013.8+1907MG3 J001356+1910?ïÎŒ<?{
U	þI?VÕôÔSÚî?d("¼ô´;?s?<Êle{?qñ2Àn0?ïÊqW¨Þ?vƒr¶?I.*ÇýµS?T«6BLÐ?w¡ŽÀU¥¹?rœów¥¸À?ïwñûÒÁ%?‡Ö¥x%ÿº?zÕ@À
Æ?'äÓ¥î4{?"˜àó0Ÿì?y¿}ÃÍI?ï«|<³m?^îÌvo®É?W¯jêA@?6§I'zõ?'>ÈÁfŽ?^8ŒbL?﨧&?xã»­;÷ ?dD´& õ?]"WwJŽ=?€çi0EB)?sšÁÙ
]?ïeÃĘÿH?‹•<Æ7í?V(°ã4/Ä?_}Dð9)h?'äü]Lûö?‰º}¸ê!.?ï:Eíä¹A?Œ
÷{?'TÁé	û?"»&'?'
»?€{³V€ä?ïFc`;?€ßO}Q?kþ§óG?W~I
epT?™–ŸVV½?€öAGN4FGL J0014.1-5022¿ï¡rDQNãÀPlwÄ\»ÃÀ:"TýˆV{À<»à'ó@ŠÏ«úDT?ÿ{7(‹9…?Á
!«¡"?¡7öx±?àj|«LI…?ç¸øaœæ?ï(þûž¿éˆ—~6fÄ¿Ù#Ìhù¿¿áÝßÊÖS¿àg"Ý—ö+¿àp¯*$–¸AGNbll3FGL J0014.0-5025RBS 0032?ïÏSÌt§?tÖÛÜn²9?K€bóõ'=?Ff6)<2÷?tæ
fI"ò?s¾
sÞW?ï)'¦R‡?¡ÿ³ø4‹?zæ0X/êp?ƒ•Á"%¹'?"?›C	?ž[ mQ?îë®-
¶N?'KÖÏ!iF?z'‹º©Î·?rö},sú?œWx=Ҕ?¦ÇCdÈp?ìI6°\?—Ïó¡ð?"Ê–?0½C?xóæ½öÝx?¸Ã¤íÑ"t?•ÈT¸1ê?ïŠke¡ÿ?ƒŸÚ*¢MÅ?bÓ.Ø.ü?]£òÎ=4?ˆ°Zåω2?'^€³€ŠÔ?íÈ1ã?¶Fj
3?—'˜+w«?«YÏS_¯…?§þ
i?ªAñ6K?î|/ož_?–œÒk﨟?z ÿ%ýÒ?}¸'÷Z?¤øé#YFN?"Ž?z<§¾?æîš×¡?­¨ËÃeÚu?¤àf#ùÃ÷?"ÆÝ窳?ϸ~ò?­7ù-¸PèAGN4FGL J0014.2+0854?æ1'³ÆbóÀJm²•éâÀ:ÆL²`9üÀ<$ü.º'¯@p.#(ùô@á~4¹E?ÄBáÑ윿¢ÀÛkT?Û¬ƒå@ýTƒ™¿ï9¡v\Ô?ïùƒyœ¤¿åñ™ O–@¿ã.IW¿ïÿùŸé"Ú?ïÿ·ÀÌ
ŠAGNbllMS 0011.7+0837?ï§AfÁnä?}iî"îuC?i(·h:?bd¯*8 ?Ë=ßP"?xøêìJÔ?ïÇ-Âl1é?vRfÿ?L£
_|¾Y?Sof-w?xÔ½Ÿâï?sÊEg]?îI0deŸ?œÚZWÞß?ˆ½öÞmþ?‡'ØG9?©ïqnU"?™Y%ü—?ïàn{nò?qVfí?`pµO¥«0?L‡¬ðº÷?‹ë·I\‰?né­µZÂP?ï0aì4¥?' ò-!'?…ðºhÁì?…h	ÌÓ?÷¶|ˤü?‡¨g'¶PŠ?ïaìpDûK?'Nރ…:z?^¯ýݳžV?k‹kË¡?'×rÚ³?"©§Ê-?í™N¨?¤öŒ\ëÕ?ì⑼Õ?ˆg&¸xn?³ââ|%?£$úÖã`"?î˜AçùEs?Žè­C"ªL?vë:ñ–ä?jÔ¢ì@ÿ?£žzÂw?Œ}üÆiÐ6AGN4FGL J0014.3-0500?àµRnÀP‹¬GG"À9þ!e«U"À;ó×Ûô‡ý@ÜÀ? ©Ù@Öæþ¸?¾á@øÔ2?¢hEÿ/Ý?äÓìŸ@ÀëNB-L?ë'm{-È¿ÚíÎm¿è¬l°{¿Ü;ŽK‡½Ï¿åÆ û;¿ðAGNbcu3FGL J0014.3-0455GALEXASC J001420.46-045929.1?ï萼·g?[EŠ0—Ö??†ƒâ?2K¢òðžÝ?cøÎè˜Ë·?Xu}ïeÇ9?ïஎsJÐ?l
5̊C¦?;¶>4/Ç ?CʟTÇX?kÚ©]t€?i*Ԗ¥y?ïk³'µ&?"ð‡¯9ӆ?dÆ	U?cWË·,¶D?ðÛõ´£?"[ýÒ2M?ïZ­e~_?mnáy ž?`I%˜æ?AÙÀ†.Œ?'¡.¡C«'?lm¹²¹ß3?ï̹&Û>³?pêš¼`?T³,YN¢?Hªi‡Nƒ?t{ÿÀkÐ?mó´˜Ò?ïÅ6;·w?‡c¸E³?N"RÎïÉ?YMâðPc³?†¦mL¡S?…'"ºú¡Î?î `»µ*ø?™êh-C?wX|Gi+?x^€Lj?£ä¾=åT?–Ðææ=1?î?ŒDÇZG?ˆW›!P?x ¯|Ħ?aÙÒleƒ8?©%ÅԎw?‡eðóé3oAGN4FGL J0014.7+5801?ÐÃrc¯ZÀþ¡]³9À:ŒäxºüÁÀ<Uò#žjº@"R·Áø³[?øÙ<|ˆÛ?Åå¥vF®:?Ɖ·ú,×O@A&PÍ@‰¡a¿ïá@Âgîý?ïê'ñ¶'!¿Ó~°_-âç?­Ì8þ#[û¿ÔÜX[
葿ߥ83M4AGNbll3FGL J0014.7+58021RXS J001442.2+580201?ímӏ?¬%ß÷A­"?gaYQwe?]²ªÐ…ß?·yÈcžš?«È­™°ß"?ëò¤öwž¦?¼mˆèˆ?Vh§<O%ª?hÁ|ȹ¨ê?ÀšÙ4º?¼ Æ?ìÌçY•ór?¡}TžÐ«£?oi)ªÂb›?^·wÁÓ­?¸{ä°vÞ?¡kkcb¤?î҂A@ð"?}DzEìw?nKYŸÍs?SÛ<$"!? ó&Qô"?}'E"@?èt'¬‡ªP?¾ðþ¸àºH?z<saEÎ?nSšœ#d?Í[Õ±ÖYò?¾²hÈki0?å&6wFš?ÈÆt ÁÊ?c"'/–ƒ?rZ7&?ՍƊœ_?È K9BÔ?èU|ö9œs?²×
÷Ȫ?}ª=tÀ?q#•'E›?ͼº<ôŸq?²°Ü¦:?í£)ÿ6?–Œ3Ýÿ¶?'fxÔ?rÇó0•?µ>óa¤?•êË@,1AGN4FGL J0014.8+6118?åÁo'p@Á¿ôr6~ANÀ9u?èM[ÓÀ;×4ÊâçÁ@ Œ€¨ô?þjbßÉ(Ó?»M•ŸŽü?ÁëvÛÿo·@líԄQ3?ý
ÀN\¯¿ëgT7¹F¿¤^ÞMu¿ã¬Øpnýå¿Ùìý™É?¿ÞRe]Qꮿè
þEjÃAGNbcu3FGL J0014.6+61194C +60.01?í¸Gù$)ç?Ÿ±´"?uUf—ÄA`?l‹k'/C?°èiÏ;6ï?žM~*Uӗ?ډ3mÉ9Î?È,öҞŒ·?›¿%ôŽº?¡/ƒåÎ?áÝmÒ¸c?Ç)Ð[Ö6?ìe艎?£&Cc;•?'_A²f"ë?ˆûKÀfÅ®?º¬$`²rY? ÷…Ùˆ?èÊ\	ɶ?›ªÙpÒ¯?ªËD•
÷B?‰ò61?Æ$½j•[X?™ˆ+]%õÞ?ë§Jú¥"9?ªÂ"…Ù!?"sÔûÿÇ?Œð"Ò$€?½è²éCGu?§¢œ,º?Ê%4æ?ÂÓrÇ^=?ž'a`Ž?¥#1G§¾?èŠå˵7?¦éV×A?én"Zía?¨f¬ŽI÷?ž;<D"}­?'¬™.Bf5?Æ~LVoÎD?¥±ÛŒ† >?ášNϊ±
?¬T(Üy/o?»=6½èi?¡IO)]òO?Õü±pƒ~?¬g'¢†MIXED4FGL J0014.9+3212?ã"MäS@À>™»'ˆÛÀ9ض쐷sÀ<^xîÿ&¼@a]Uñy*@}_~ë˜j?¶'+èç	º?Áú
ø' Ï@5µœ.ŸP@¶`˜Ëþ?xî(g¿â–NöÞO¿é¦'™ð×n¿è€åM¸¿ï÷™)1Q²?ï]€C‡>MAGNbcu3C 6?ïöNÓoÀ?J?ÊÍüÀ?9V\•ã?DC……·B?J'ç2J?<3Ñn?ïÁ%ÏñF?|ªª_ýÓ?TU{õ~M·?`Qc{v­)?zW¹µ
v?v ×Ùù¹?ïÀ7èúã?l;" Gs?Y*ýŖ4N?J¯ªú÷?y™L xÉ%?iî	½ìÔ?ïà
{?O—}mÏ-
?Y_¿9~`?A´EŒÎ¬ö?cM`+žõ:?EXIoñ¿?ïírM
°ï?UúÞµ"ë
?M!GŒªG?JÙgËÚ&	?VŠÁòΞ?IÚ#r"5ó?ï>ងԪ?š¤ÑW·Q.?jÄþ Ò'?†iîÉ0fù?"Ë,T?ôí?"¥šóz¥?ï–Óæ
zF?xa@¿:K?fóLL6ŸÜ?kÒåÑd»Þ?"Ž3uR†m?r1äwÝ?ï"z—í?rm2'ô?võà"'gK?e^J	¤Ê?'â$M>Y?g¬ø+ÑäAGN4FGL J0015.2+3537¿©£·­:g-À:­qGÏ¢À;x–z*h‰À<Í@N¤©@!8ÞZh×/?ÿKùƒ<Ú?į	Bsí㿤ä¯þœ
ù?âAªŸ¦N@¾ÌY	‡¿¦XåIpag?§‰\¾$›ô¿é§h5"¿ß¼MΕ¿Óz۞ ç׿Ö±MëE^AGNbllRX J0015.4+3536?ï¸ÄgM—
?uÙó@Éݦ?Cvïy¸¼>?5R͋ %]?€—w5ژ?uZº<<¿?ï¡SÓu¥?"JîW?W»gÝzh(?aÃÎ+KT?"³ž,Å=´?š,¦Ñ	x?ïeÈbɒŸ?|ÐqTӂ?_òæRu?_+]/ì»Ú?'J¸~ïƸ?zRÅô?ïOâã±ã	?{âñ_$éô?ZPf´dØ?Dâ‹x®[?"^Uçh?|']אd?ïuwÒä,Õ?…Cm…B^?U2þçõoË?MY¸zŽWÖ?û«jNã?"[ÞJh!?ï²oÜåQ?—<Qh']?fWörag?qÓ²(˜7?šÞ³D´'¢?"ôíâ¢ö/?îÛ|R‹é?Â'Û6?cóË+qy¾?f¤ÊP£âð?¡þ"ҊH?Žz5c)¿?í}—Sj*?˜×r«Ðá?v4èxҊ3?l©¼Gà'•?²¯öÜ5?™ˆ—F8UAGN4FGL J0015.6+5551?´(¾ØEæÀ Õ}uv¥À:-ñŽM5=À<@â
K³]@!K'Z°Ð˜?þxòZ%?¹7ʜ›×Œ¿p÷B"ÓÈ?¶6)Ôº­@´€Ǒ?ïþrÎ\¿Ú),VJ¿âôÿý²H¿ÚP*¥Em¿Ûšëÿ!Û¿Ò£'™¾-AGNbll3FGL J0015.7+5552GB6 J0015+5551?î1T!{‹ù? [eÂÞ?a˜•Û'?hPYÈìíý?«Ñ=0eR? 'ž
˜?é[A`·>µ?»VÔý˜?bÜ£™Ì"?kÞý¤¢d?ÊG‡ïß1º?» ÄÌx>?í·õl—ó?˜Zõ0¸?vIД¸¨?p¤éûÒ	?°ãKL™0Ÿ?—˜Ûê³"é?î£8LUK¿?iƒ]d?tOc¯˜¯?S]ô)k‰ë?£BŽÄ?–?^+s'+?ë{zŠ¾=?µ[³6Ò
Ï?rÄX"»c?sNÄ,?Á{õºí;?µ1Ęû?áÕÏ(Wô?ÄñJ+X"?e{û…¾6¯?s…Mâu¦?Ü)i¸LÚq?Äåèâݹ?êNa:58¥?©‹øùÔ×X?'±®Ùü?uŒ9Ò9>T?Ŧ_û"3Ï?©#—O`'?ìÌ4ÿð?›8äþó?©_ºn´?vQ(‡Å?¼D"v>B'?œmî¯ÔAGN4FGL J0015.9+2440?î=Avö_ÀB¾µ²ÔÔÀ:Ñó¹À<~µI"ˆÁ@ã&T'Ÿ@ç!éB?¸@ï3t¿±¯Vš@ˆ†?ù'KiŠÞ@ºÄNÎð¿ã|VÝÝ@b¿èÄ(Lýà¿æ	¢–"¿Ú0±CŠÏ¿æÕu³
ƒè¿Í¦ÙÉ	žºAGNbllGB6 J0016+2440?ïä礦?bÛlZŒ¤?8æŒf(F§?+ë
ÌÍÿ?há•å%z?b+ÄEëúÁ?ïÑkm¹R?qˆðfFfZ?Azðü?G7ìyÇ?u-bû¬?oë 
˜¨?ï" S ¢?x–nþý¬Ø?Um+ö­ó?I¼U'Kì?ˆŠV' w¼?x	ÇQé`?ïŊÄû®H?['S™¾¢?OÞU­-Â?4Ù"']Ü?yY¦®¸?ZuyÉ®€û?゚<h2'?€OHLÕÞ?LGïÙ	q?=;Ïœg?}'q­2þ?¤Ÿ<áÔ¼?ïg⠊ÓÈ?‹&[™.?Qÿd°øë˜?Z¦/¸€?'ãÅ£L?Šù $Ô?ï:t‰Ùw?ŒÝ¢?×ò ?b~xÎïL	?^¯áë…¡?™èâW"¦ž?‹¶_fܜ½?ïG,#õR¨?|·)à>½­?i'Yoˆ¨?X>·¼•€.?"ê0U Tü?{sô+$ÕAGN4FGL J0016.2-0016¿î+Эï‰ÀNí$ò'Ð)À9oßÏpÀ<&4ú³å@­ã'K°@èƅŠîÜ?³{qæLOº?ǨƒÂAÙi@€8AíH@¢,**uõ?»\$š¿	¿åÿ$£Mw'¿èç6oþ•¿î´w JŽ¿àŠB
ÁŠ¿ï¼=Ó %¥AGNfsrq3FGL J0016.3-0013S3 0013-00?ïôBäoðm?U|&HÁsS?Cp/œå:?C?ó­|h?K">©ŒŒ?Lõ3ð&ú$?ïÙ­ikd¹?{ÇÈ=µY÷?FE˞X'œ?aHª"ÄÂÅ?p`'Ü}F?u
iÿbÍ0?îõô[匕?•$•ÅAÓ?€±@AËÏ?ƒó·•«"î?˜èÔh˜1õ?'ªþ€TøK?ïÚWŽK ª?Sçñ?Kœ¿Î=Žw?:̚-ã"?nÁA©B®ü?O `þ(ÏÏ?ïé_þÔm?jŠ~7'<?RA	»?SQh¡ØÄ?[,d'Ö<?czæWb¿?ï‰ã
@?•Ê]©ëÐ?aVNÙQt?~Eh¯¶Ð?‰f´¹{­?æ5Qçˆ?íú=F:)¥? ðB6 ?ã­+JEC?‹ŠM£^?¨ã@Rf»\?œ5ç•x?ï‹Oé?u
i*'$>?g+¥VX³?[VQù3Ï?‡oeü#Ì?q·»qm›AGN4FGL J0016.5+1702¿Úª7h™hêÀFƒÑ¼râÀ:³dÀsøöÀ<j³fÊ9@0ù¼‡°@€ºˆ&«?Òç@ìY?Ó¡$'|œ@Ö_Æ	@[Õì¿æžï!‹k¿ä±^ýfr¦¿äì['û¿ëÇ4<G®ë¿ïÿ!Ÿ>õ?ï÷ZtÀœ=AGNfsrq3FGL J0016.5+1713GB6 J0015+1700?ïqÎé "I?…ïܼñòÓ?edw#S?[òBÐNªe?Ž3'Åwá?"YùèÜh?ïyã/K?–Àè·Öu?fOmKÀòF?qFRzñ?Í?Œ*kë3àÅ?""¸"é?îÉ,CLR`?"º-69ºñ?}/»Ü÷?}w°k8Li?ŸŽˆœÛ¾8?'§e¼_|?ïxá¾ ?km]ÐdŒÀ?Sûn2$Þ?=Ûçz(·C?†"Y¾"¬ð?i¤¨#ž¸a?î«"éï?¢lëC˜º?r'³ã— ?kø' G?¢ýˆ•0?¢&ß|w«Ð?îÊ 
bOg? ÁˆúN¶?rºKÃÍu?{§à6ê€p? þµÇˆf?·õœœ$Ü?íâÉ¥iË:? «b˜W?"C0ŠA!?ƒ£r¢h,?¬Â™‰|¶¢?šÏ"£o¼?î̒)ã©2?Œ$1På3?eŸ9ª:b'?X33ωlZ?¡Üéɉ€°?ŠÚÌf`â7AGN4FGL J0017.0-0649?ÞÅÄn.‡ÀQÙŽuyÀ:_ŠªŽÀ<`íjÒò@"†qsµ¯@9^Æ^ô'?·]HZŒ¾j?ŸÐ‡†5}?ægf
öÔ@
63ÍÔ?ïʇ½ùö&¿á#W¾,öÙ¿æ	8æ0¿àéT "¿ç6
]ÑíH¿ÛcS!DAAGNbcu3FGL J0017.2-0643PMN J0017-0650?ïîw,n.?X3tpp"£?(òöá"?F*E>í?_óHÍ$f·?WQcÈÅâ¾?ïè™­F?j}&¿	Q?2¦™¸r©?@È´Öü‰î?eû_W5?g¿9š*è?ïÁ4ĉ?je5¡
x?Sõzô'\?[C°ð'ŽÈ?zh Q»µ?e*Ÿ¶H6à?ïÖ:íå?Pfg3‡?J—°¦íµ‰?,×#ÿ±8|?q"Z·ñ?N§@×ѯ«?ïßjÍdˆ|?a8ÅUùs?:<.?V?)ÇCfƜÄ?mR+ ‹*?`Œš¡r
?ï´x-@Þu?ƒßá(×?Cxçg3?Q*â»Z³?©Ý"Ì-ú?'•äMý?ëÁ7K?|Æ£'äÊ=?dz½ÿ1%u?sÐô]†Î?"q•"kß?p…Dkmµ?ïxûY?l¤`£Ø¡?bh'È4HD?NYÁúß?‡G "ãì?iÓÇô¾ôAGN4FGL J0017.5-0514?èç˜8gGÀPª½Qï·À97@´%6À;ۀ
×Y@㵈b—@ÀÓ¢±p?­xm'—ýì?ºé'9Xç@	HdóŸŸ@ÁI©lJ?Ð]÷ÂnÏì¿äŠ&ßè³]¿è-©¼&Œ\¿ér*ŸÔy¿ár\=îx¿ïÿþó…õAGNFSRQ3FGL J0017.6-0512PMN J0017-0512?ïé˜ÉKI;?£¹À"ìÕ[?@"óSˆ)?{¿?O‡
û?bEùîà¹? AãNÈÜ?ïñ±PÎ^?cÉèW?'	=TSÄ?9ì|ÃRÑ?Y¼7%øŒj?aY4çK?ïžóJ1sã?{?·jÚÓA?`á>´É³V?b?ÛÛ.¬?"
ÝÃXô}?yÓÃÛ½N?ïî­ÌpJZ?DØ=GB.Ó?.G¯€Ÿßµ?"_?§D?^ÛqYlõ?D
I7(Cå?ïù$ód?@Á˜Ë½u;?(ƒ«Žî(À?!˜ôh»Èƒ?EM
<0WŽ?=r€"T~?ïÉò+I?€µÛ[`
?Btöà'6´?WÍ;ÖD˜ª?x¸W‰Ñ'ì?~x·&ÀY²?ïPm‰Mú'?‡öú€‹Áð?m*|W(k?phå5"#£?'LÿO:¯?…d•€Û1¿?ïȤ"À;?föýI'°?LGꨍ??MçÌ-?x+MPâ»â?eûz­}¢AGN4FGL J0017.8+1455¿áZ3ŸŒÀG•{t¤ÓÀ:£ß\òI^À<‰f1A@s~"?jN@?L¤?Í_,
u?É$Bjۗ?ûqG6w@<¼K <v?ïý?ѧ¿ã/+f¶¿à("` Ò¿àøý!©H
¿æ6""Ý¿è­-]AGNbllGB6 J0017+1450?ïˆ?¯ð?¬×±Î¶à;?p˜§tÚ7»?«J%ŠO»?…«ÜVÔ ?"Ks°v¶Þ?率LJà×?~"¾î†¿?X-Ñ3‹¶?X"‹Fmî?ƒ'Óøž5'?{õ(¯£Q?ïf(A×Tª?{ÂÊq‡¾?h»§&p:N?iñô®!Û?#'è²nm?w÷úHó?ïBŒaÍ¥e?hÈÒä£?iÖ½H@Ò«?GWµ­N<Ü?"sœçò?gK;ž®Û?ïU"]*ä–?‰toñÉi?bü—Ò"p·?[>[‹é'?'íáZÓ&?‡ë+8'6·?ïÄÚ1†­?"OËqo–?hS«Ûs?p f5?™åÚDA"í?'Q™ô?îàaAìçþ?Œÿ2[ºv?uŸÒÚ_1ì?uaµmÝÈ?ž‹ã
—VË?ˆ90šžôš?î'B©·Ž?"p¨®
Z¹?y÷ó˜}?b5r=Rp?«¸ùõé•t?ƒt?G©ÚAGN4FGL J0018.4+2946?ÌÍfŸ5(ÆÀ@F-¶°`À:[ŒõFhšÀ<RùôMDV@!JË
)úz?ù€ÝàñG?Á*Á_0g&?ºäeb…[?ü}w$#Ë·?ùjž"dÿ?ïx³ÀŒLª¿çHº•"<¿Äê0_ï(í¿ÐQõ–²Y¿álîu"Ó?°m®^kAGNbll3FGL J0018.4+2947RBS 0042?ïÀé>>÷Y?pà}ùÑ?>ï‡@¿(J?,>Ûðµí?}œhhŸÉ?o[ñ"یÚ?ïQâî¢4ž?'C8`…#?pŸ]Z#?s›Å'™Ä?'›ÊÛ·Ê}?‹Åˆf¿Q?ïFQê>³Ö?':¡q–N˜?dÝÆu,æ?]œóR1úô?"š	þqå"?²™mÃ]¨?ë®+Æq,Ø?'ÿÐE­R?ŠmãkmI?iýÓ/àhñ?¿@å^¥8?'-Q­Œ?ïJüØO¯7?Š@:ÐÜ?W©ÇE˜ S?Kâ›Ýa'Ú?•%ȇ/ï
?‰¡²ãY»?í×ð?Ô½m?® 6Ç?…œ±Kóæ›?%Ո¥Xÿ?­Ï­ÿa‡?«»>aèè?îrùӠÑ?"½­üÑB?p'9ýø?f‡ÂŠç?¦ÀB6'?'ÿÍïÑM?æPÿ³H?¥ü\Þ,Ž?™s´g'?ƒ–­F˜Âc?Ò6VÅá9?¥ÅVSŠAGN4FGL J0019.2-5640¿çÇ>­å«ìÀMòÜ­¡À:m'§7À<³[bý%Z@C+xÕ@_±%§Yv?º ZmO?¤-7#`_ð?éÔò5<!ï@O•¿ol¿ÂסçñÁ¿Ó§ŸÁ¦Óê¿åܟ]}ß¿ÜPLßÖë¿ç/§Ã(]¿ï¸uý³¦AGNbcu3FGL J0019.1-5645PMN J0019-5641?ïûx³^Öi?G:yŠÇÐ?c@xúü1?ÙîxÁÙ?>¡'õ<Ë|?Dœ¬Ã÷Í?ïð.˜2«?d"ŽÃtÚÙ?(¡Â¦ }G?9 ¾Ê)?\Ž—›ß7g?bfýŽV\"?ïÉw¦¥"?bdÊ
IâÒ?OîQ«T¤?7#Ï(ò?wFT~V¥?a}/NÃ!?ïøÔöùo?0u""\?ÿ^E
 –?o€âý+?IŒ8Úܲ?/	¤ÍÉ?ïøÏTLÅ?T|Vñ1
È?$Ÿœq…?+­"o ™F?HØÛ!â^æ?QDýøù,z?ïÓWÏäs ?}Ž3ú£^?6O;œàÈ×?LÌ¡PËe÷?tï$j_p±?|M'Zæ?ï¬L^°î?p{ºRÐ1?XÀŠ²À˜÷?W4œ:Åæ	?çۗ#[?m{֞0yê?ïîh¦©ð?K>¯ð6çh?/¬ãô91?ð–uŒ?_ù'±Õ›ð?JßUZYœAGN4FGL J0019.3-8152¿í7™VÓ¡RÀA"¿]xÀ9µo`
+ÓÀ<IîsÂ@N1‰9úù@šbÞòi?³f"nd6¶?¥B<Ä	7?ò@‰ƒœ@½×¿â úa§°¿â%\°Úÿ¿á}Gô‹W·¿à\øɪÙ]¿à×~0‡‡¿èï;!>>)AGNbll3FGL J0018.9-8152PMN J0019-8152?ïç#`_ï²?Z;ŸyöC?:š'_q›Þ?+gæ;(Ÿ?e‰M1é1‰?WÇIªªy?ïÑnÐZ?u¡ÆC…¸ª?BH, ÏP?JŸ¾ß<Ó¨?u.Ö4Þ?s¢
8‹ŠT?ï«š¥nu?x+鍮Ç?T†€›œ'E?@×ROs†˜?'®I5ÊX|?w¢É•I °?ï—_s"2Ž?d·Dî·?\"Ëyÿ)?<šç$^
1?†•©Çz'œ?cSQ}¢ug?ïÉzUþÝ?páãˆó©?OŠ´Ó.;ê?Aq–݇ô?wNìGt‡^?mñ>wY/Ì?ï]è"¾›Ý?–öÙ`^?TÇ,+Ül?e꓅Ñ	K?'öˆíUי?•Úo9ÙŽ?ïaY²ß÷Þ?…ò–…A?b]̖sƒ?X¢7Âuñ?''=榣Ô?"¼È4ò
?îïZ™‡?'8óEð?½?r°…+C•?\,Þ8¿_?aý·U‹0?€ú¢ÄͼAAGN4FGL J0019.6+7327?Ô
zí±ô¯@%sõ/ÂekÀ8¬ÿ˜Ñó}À;cgž@–×í<X÷@ÛVà·e\?¬¶áAèœ{?²ûðü¬äO@Å6B²,8@DVÇ?ïÅÒr(;ˆ¿á
/þËLš¿é1rEî¿äõ¹?§4ã¿ï¨ÿ"_{f¿ïÙzé¯AGNfsrqS5 0016+73?ïèémÂPG?]uVlôw??Ù6+3'º?5½²k¸5í?ck¨†ý¤?Z×êã
V?ïÅ*¬jÆ?Š"êRû—¿?O@(²¿Æ?b[|
ç?yˆXáü¯?‡ÿat4µ?î¼9\ w?–ï	5ÿXu?ŸgA‹CH?À'¸Ì%7?™© Ë&¯l?Óƈ
v?ïÅ2&mÒì?_­ú8f?Y×ݖXzu?C:€p@ª?vðõwn'!?[Œè	)ü~?ïÆ_ÅYÞ:?qKj€Š%Ÿ?SõSp–É6?Ov*]…Ý?wÒÈw›?nÝ®è§q
?ïqÏ8
û?•ÈÎßxUd?f%(IÃ?ƒþ»}Jy?Žîzz"9?'ýsÈI'a?îSgò
Q›?›=¡¢ÜÌ:?"™¢Ül?:H¡¡â?¡>´ȗI?•z7EêÚz?ïOÁ¾É ?€]`ýŸ"7?wíœûIÊ?kt²˜¼Ï}?àŽOØh?zjÈT#äþAGN4FGL J0019.6+2022?ïbSßG›ÀDð\|ؙÀ:Z°,ƒÊÀ<|à"&þ@»½•LWò@è"ÿ‰;?¿Ì[㫌?¾[Ó µ'?ü§›4¤L{@*Ò2<h;?ïýròe㊿¥}¯-T¡î¿âë}'üf¿ãٔü{ç¿éì×.OŸ¿Ôܐ¤¨koAGNbll3FGL J0019.4+2021PKS 0017+200?ïÀ¶âæÐÀ?mú'Ro.?Y¾¢u?Wä=sRXû?y5	G_Ž©?h¸ã"WÅ?ï¦4PÙP-?€§¶2™"Ã?Y–‹–ó?^>¦mïõ?ƒ@`¢+â?|`€e™v"?ïi[Ç.°Ë?ý3QþÜ?j9¥ £?j:|>üƒ?#ÿÏޙ?{ÀWh-¦*?ïeTâÅu?hÁèDó¶?wEúǚ%‹?T™Šì\Óù?‹Ê
ø?e©×ú]#?ï]"/-{J?Š»ûËTÏ?{ªöˆ÷[?"~ÉÄ
¯§?ŠÅ¸÷Ñßæ?yžæª*uÉ?ïƒgu|{?"ƒDÁÆ¡t?kÀe°f?tÖŬą?œL/9›°Š?'ó$'‹?îÝ€˜–º?Cë£b×L?}?ǃY‰?~.c휚e?œ÷¾+ãøQ?‰Ô"æ槵?îjaD¥?'êËj>
µ?<Íò®â?qÝ-Zt?¢ k²åø?€nÄ3rAGN4FGL J0020.3+6919?æRÄ}?hB@·¿ŽaÀ:>TÁù44À;£©8s@ºy³ +@ËYÝÁç–?̳*yÑ'O?ÈOÊB®Ñ9?ýóÂî?ãË(²H3˜?ï;ØÞ¨íJ¿ÈʺÂH¿ã¬Y?6vµ¿éZoíÎ¥¿ïÿú¡œGt?î  ¿'ȜAGNbcuTXS 0016+691?ç7ùï£D?Ȫ€Úäp5?'î:µÒm?'WqC¾?Ða(v87÷?È)J"¼?ÛܶAù}8?É~¤î?¿rÛÐÜã?»0N"ûÛa?ÜF'ÉÏJ?Åo¯#?åaG³üNù?±ÔyYL?©¸½i`?–øÝ^'?ÒXëdΝ?¯ÿb²‡?Ø{°—"bó?¬e}ª?ƀaòâ	?£´h?îþ1?ÜDoy,?¬%Ë%3¿k?áRMۈ¯ð?ËqOãíûœ?£/v³b-ø?£´)Ù;qÐ?Úõur×A?ÊÛÎI›÷º?Æ䠊ñØl?ÄA' ðP?Ç9-0?ÄÐð8óÍ©?äI—´Î:?Æ1'¹8?Þ0¼Œsýd?²|cê}eE?·ß>&qÒØ?Ÿó¬â+É?Û×sê]e?²¡}M9˜?ÂÕ	c3µ?¤cakµ?ËФRˆ?²‡HF0_?äV±Ô	=R?²Àsh8•ÌMIXED4FGL J0021.0+0322?ÂÜɾ">«ÀMOÀãŠ~tÀ; a3÷~À<™A<á1ß@ »ÚҞóÌ?û6ìü=?ÐMØ%–¯?€Å'pÛ?õ<¸gºú<@éä.b?àI '–ó¢¿â!3E¨¿äp¹pÏuô¿Ïp-åk*¿Úaj~#Ž¿æ`–
õAGNbcu3FGL J0020.9+03232MASS J00205023+0323578?ïîÄs·Ý§?Mµrœ½i?(Ú1L
'?"ÿoè5£?_[ÒÐN6ò?L²gš‰?ïؐR¦ž˜?r_¥bʊ?B	<"WkÒ?K'ÍÖÅØ?qv¯>†uh?p

K%?ïš[Ղ—¹?p]Ý2Sè?QŠŒžÕ?5þïï?‡7¹)׿Å?oü¥²øt?ï†î'	?glM"u?Ae
ðªL?(|ïLþH?3Éjž'­?f¬ƒh:n?ïÞóÞè
ô?^Eã­ò"?8‰A;›X?)ƒ3DKª?múù&®'?\œ^"Gt?ï•Waž?ˆßèċF?O°'
P×?\'D`%³Z?ˆ¯™¦¸D?†Õ¥óËèl?ïCk‡í?^óZ÷¬?UÔå¬aV?FèPkØ¥"?–5Pa°U?6(¯™Z?î¢ØWDŠt?"í«u¬W÷?QÒæëԞV?E%$>—´³?¥CãU`•Ó?"äþ±ÿˆAGN4FGL J0021.5-2552¿ÝÜ*¸»GêÀTÌǎŸj"À9¤GOIê/À<WëÃ¹ÿ@¯mŒöH@§¦tso?°/R¾hÛâ?§ùâ&Â?÷$êµë߸@#8Vˆ¢Ñ¿ÞgÃ}î˜O¿ÛyáBz£à¿á$ý°šg¿àl°Ý­ð"¿è=[‹`œ¿ÔÄh¥/úÅAGNbll3FGL J0021.6-2553CRATES J002132.55-255049.3?ïòî?kÙK?HÎT8a@?(`3'ØL#?¦ŸàŠÎ?W{"´U ?FSf3Œct?ïá_xi&?t!CÒ~Ƽ?8½Í>Ûn?Gd.=ü@J?kàþÜä!ö?r'²»?ïÃî
S'?o¹JcLh?S:Vl8"?\W*ÆÁˆ?y:w‰Ê$Ä?k~B¬Ÿ.?ïÔۍkB?SiÕFÔ?GSðèÁè?.#¢«©?r±NàA'"?QÖËã÷–d?ïâH"iȂ?a›Wãä?@™ºôy܀?5ÿ¶Sª+ß?i'nés÷Ì?_ëû.;ª	?ïŽ9.÷<?"tÄϲ˜4?P{ f`´Ü?`‡µø?ŠbPwÔ²P?"ƒÙ+}p?ï80aá`?ƒŸ5™Ð°6?]ͽB'C?e8ÕjEe/?ˆ8<Pv¶?'o;´ê4?ïœw–Í·?q/-> |ð?ZšƒÖ'Š?IR€x'?…ŽÊi#L?om6eŸówAGN4FGL J0021.6-0855?&ó="£ÀQžc^J8À:÷ØcÙÄ,À<Ÿ#vý_@Ñ£žU@@DXÍ?Ô5lÉV÷?У–r¬?ûü'¶vI2@£&T'Ÿ?åð ±»ÏO¿áv+ÀÎð¿àvÔb˜P™¿æ.Å_ñ_¿ïÿþÐñ¿îkV斢AGNbllNVSS J002142-090044?ïÃ'2?qã('ík?cÙQ2Ý?^&!PmÍ?tú	,ä¹w?i™)c?都QãÍo?—D^bŽ¦?aþº&HU?d÷ÀË÷Œ¬?V½
"Ö?{ìÿ?¹E?îšÎBÌ6?•s:ˆ‡»…?'¼]tík=?·iäNÐ?™éÚ3C¢?‹"rÌî^,?îí
;Ä|?wùï?Ÿou?y</ûU)]?_×ëÜ)¥?œL›†{&?uŒÑÊa‡_?ïiX¼¸5D?…X¡îç?y9ÆIìV?t²¥6äKL?‰
Ji¦Nî?}v¥þsº??ïu	8Û5?š›QÒ'?tñgò9¼7?"o*á··?—õÞ½äG?""!*_3ž?íæKe¦ob?œ gR<?˜ oè{è?'t쥫ç?¥K®¯ë?"L¸ÜzÌ?í"O¼Å‡x?''".l\Ç?'ì1f1fÅ?v¯%={
?°ÿûëÒ+?'ãåê–f}AGN4FGL J0021.9-5140?ì³DSI±­ÀP5w ÈÍdÀ9¼•*™1À<i㤦©@ž4E,@m^•—?°F¸ Bj´?ƒ—»W¦Ò?Ñ}0'S×Ã@cː6Äb¿Ætž7ŽÇ¿äÑå©és¿ÞaOÛàf¿àLJžDy,¿Þá\ü°?M¿áñŸ,ݯAGNbll3FGL J0022.1-51411RXS J002159.2-514028?ïø™¿â·"??ª·âR? ³>Huz?6h™GƧ?Il0Ÿç&?<3á¢d?ïð¬xCˆ–?e90<ˆ?$Gµà7$?6–ƒŒ\?\·	€­?c''Aå…Ý?ïÆKoÙÆt?lï‰vó?QPÏð%"ú?`‹cÆWùu?x†&1¨Ô?g-‡ˆ""V?ïî^±5?B4¦˜É·??-¾='=?…°œH˜×?_‹úò¿m›?AâÚÕ?ïñõÒ:Ü?M‹Cž;;L?1ç©ðe?!ƞI³X^?Wš" ÌéÔ?JÅÀ}3¾C?ïÎ*'úM—?~[0ÑyÈ?6ò	î¸ô?I÷ÀÂG
 ?w{˂"ÑU?|µ)ºZü?ï¥ß6çj?rKZ‰ráÈ?V_Î2Ü­â?]mþI•Iý?ƒ¼C#S‰Å?o¾ŠœSÒ?ïؖ8ÞeH?\™ã:RYe?@?6mú]?/Òk¹‹?q¬ü̾ë?Zù
Wn¿7AGN4FGL J0022.0+0006?íÒ»ÀÀNí؃º4DÀ;/…(ÉÀ<~CvwU¢@#zISž?ù;ë2éaX?À2AƞàU¿®p——¶Àq?ï"{[>@×ä"Sçß¿ï&%z
?ïþC¢|l¿äVÇ¡Р¿ãȑ¿/«>¿à@óæJ?àâÙ,,¯AGNbllRX J0022.0+0006?ï»sp\€×?ƒvÂۙT?4Ý:ÃÌNG?2æ>PYG?€|:	™Ý?ƒ>œ³€{¶?ï¿áb8·à?"ðJ%I,ó?TCEuFš?hº*f»ŠØ?zþ}Šùzv?€Ÿ2}³6‡?îù'˜ GÉ?'ä.má?\‰VY–²Ô?ZMf‡=âg?Ÿ—
‡¯?'Ù(›l¼ô?î2M"3©?™"jw9?gZ§§2Ž:?W€öe\Y?«e"vO
?™"š‰â"?ï‡*Ï–a?"ºAiCö?F¢Ké³x?>ôýÈö?ŒË+TEP?"¤úhú.?ïVH«.[L? Ë-Œ€<?f՛DÂçA?¢âÇKµ¶?'\7.,Ÿ?œÅ!îÎe?îw@Å(Nå?˜]h7:/?c&2[×H$?cy	—'ø?§Y‰w¯?˜'è@4'H?ꍵçÍ?´Í5¦ «?€# Bùû]?~É¡Ðóî'?ÄÆùïDÆÙ?´aóÐß»nAGN4FGL J0022.1-1854?íuU¼
ü‡ÀS×õY³Ð}À9Ÿ‡mG+8À<æ¾æZ=@2ý2Ys?üI(gþ?´Y¢ž%•?ºë¬ "ÚÆ@¼uf´iÿ@#¤^º?î÷*¾ðk8¿Ýµ‡9᣿ևî@¿ØM´ÿ%ºz¿ç‹^Öw¿Òl"h	ԕAGNbll3FGL J0022.1-18551RXS J002209.2-185333?ïÒI{—c?o]u+œ*4?G\c°{d<?A™cY«+O?sï¶ön?l«ÃÅîˆs?ï·œ	?ˆ†*£_?]#²E¼®?uìa`lÐ,?}'',ö'Ä?€ì1Oƒúå?ï<¸40ք?Š³ÏEŒ?rÞt>?tfÆÇpàœ?"â´‡ßòi?†'U÷f%?î×¹—æ¼?€nî_íÇ?kâ⨡2a?Q%í´%Ç? Æ8YÉÜ?˜œô¬?ï´$Ôíúç?wïÖÈW?YñÑ+ê´%?W¿,3»?q!-‰¿t?tZ|®í`?ï7>~šÎ?›]Q¬Õgy?pÙ¬Zÿ?~V*Š^?"áïÕ­Ÿu?˜Faq½?î«Pž®?•µ"…•?€l‡öÎ8?~èÓöÝ "?£êJ'?'›#óªP.?í¡õ†‡÷Ž?—÷nêw
V?x1µkô{+?f¾J?­+?±m8rÐ;ž?—¢L÷HòAGN4FGL J0022.5+0608¿ïòü³‰ºÀLl
oTLÀ8Ÿ6}jŽêÀ;¢OYÚg@û£è§ô¦@|\qðÞ?¤ "ˆÞ`s?ªMúY
°@8ÑØ¥H@F_Á܃ϿÃGw£O¥Û¿Ý¸¼yBŒ¿ã7õfI
¿á0[è^"Ë¿ã–#£Â¿ê
©ÂÉnAGNbll3FGL J0022.5+0608PKS 0019+058?ﶘšÖ?™ïBé?¼\?Bàuà–…?]ÝhK¦ñ?+Ñûõº?™;Æߜ\?ï㽘ìu?pˆìM.f?<Ž98td?Q€Ç(›?h°Ÿêöib?k "v'?ï_"õșŒ?*踚ù‡?gC3ì¬S?uˆæƒV0?'&úÂ]Åô?Œ‡i©,'Â?h±V?i–olñ,?Lúk»©bA?2²ógµ?†¨°¬¾a?h*]Ü]I?ïpՍ¡Î?©ƒAt†¾?MŽ˜ƒÌØ%?HօÝl?øفLW?(ò´à>f?ïµãë*?…$ÊKð?N¡X#ù¹î?f)M])F?€Ðñ'`X`?'âȁ›™?ïøˆ½S]?'éD—†F?k{%Xˆ»ÿ?u¢=Ñž´?˜'Š9Pïâ?'‰ŸM##?ï6Ø}ÉÉ&?'dT¥Â«?^1•›R—U?Láõ1©ž?—AÖïMpÅ?¡°®" AGN4FGL J0023.7-6820?ÝÈoY÷eÀHJ"‹ë[-À9òóú8?âÀ<' Í|@þ¥aùÅ@›2öÍ?µp(.mQ?µ áL
Ł?ø3)ø÷Î@Gs\/¿Ðj@ºˆ'¿ç3®eÙ¿éès€¿åÀþŠÓ¿ïÿþÐñ?äñ*å†×öAGNfsrq3FGL J0021.6-6835PKS 0021-686?ï‹M•Mô?½Á9
ñ7ï?œT øúÑc?½Ãvf'–?6S#®a‹?2ށ˜?ïÎ(èo?y·¿R"9?MŒœ±d®?aÃmÍ=Øú?u:jÒu?s¶nJ@?ïÁ®1?q'´úqt?[¸

™{?eŠYm)-1?x:õ½d"?j)6Y'>€?ïðÞ7;?Ae]{ÄR‹?HÃʪf¦?3Bg›ÍK$?Sl^&–·¦?8)‡''¶?ïÙç•%¹?¢š«»¥Ë?q	_@ׇx?¢¡^[–Y?@±'\ã?:G"ârw?ïUù<¨Ž?›×l\ q¢?d"®:dz?" NæÙÍ?'¾GÕªâ"?—^°]­©?1Ž©?zàk³×Ü?dKþðóŠ?j@n
.{»?…-쿉Ø?ulYKtd?ïɉ=xRï?gÜÍ+ZŒj?h,÷75¬?[ª^öøõÁ?nIËp[Ë?^Õ%šAGN4FGL J0023.7+4457¿u…º1ô'²À1¥3ã\[KÀ9¸AûMÀ<PZUÖ@ôrÏ«Nx@aE•6?²»®·Ë?²ƒ:\9â?þ/ˆØ6@\¼üË@?ïÅJŒì-¿ã¡Îò@û¿åÑ瞊D<¿æ‹¡>(¯¢¿é8}¿H€¿æ_AtyAGNfsrq3FGL J0023.5+4454B3 0020+446?ïñÁڑ—©?J.ŸmEg?+Ő7¸ãE?¤*ì.áf?Y˜¬Wã÷?HÚ•YêÑ?ïï¿ÊÎE?eµVrU?.Î0(öÄ?=O™.[{Z?\¨LÇ­Î?bÑ!c.¥é?ï½]ðsô?d]KÞu‰?W©(Äv'?DEwcõý"?{Œ]¿£lu?b<˜IPî'?ï셵ó'¼?AÜ[Ò6?EdvRn&?'Aâ_C?\B†ªÙþÔ?=bv¯ç^v?ïâvêd"±?[=Òøgˆ?>üb~´Â¾?,¸i´À¹´?i©‰€Ž²?Yºs¹˜5?ïɵ¸€†ð?hœø†ª?IsœÔ6û?X€zôÈÖQ?wöÃ
)âé?}6¹?É9?žþÄ}?xk("w~?h0!ô\Œ?lÕKëø¡f?‡±J‡°?rÖ<Û ?ïËEÚïi?a)TAˆ§?^u¢=­º?G@'f²C?r¿Îþ¨‡?\[¥Â¿}AGN4FGL J0023.9+1603?ïGDRÀG%ƟŒ!âÀ:"¬ñe2ŠÀ<s
=Ö$@É­"£:­?ÿPœÐ…¿?ǸÖöœT	?ÀxxšE'?øZÁ¶%@S$彉Ž?ïâHZ⥿ã#˜ ö/G¿àsÉøÜö¿Õƒ
¼õ¿éÕ	ÖB—¿æòçHy–AGNbll87GB 002122.5+154553?﹚oó¥?pæ4'%"?UЪp!?Lok·ó?}¾ÓD ö?nxKm ;?ï›×ADîÇ?~£xNs%?_K "Õ
?aà‰
ùq?… ˳g{?yzè­î°5?ï_'8T¸È?ƒ1kweCÔ?g@·ÇTWc?i#nüVb?'%½l?'%vU ‡?îÙ^âIÇÛ?u,XÐ0?}FV
â?[jV¬¨HÃ?'Ž8ˆ×?s׶%…?ï[¾¥ÐQ?ƒŠ†Ã1zB?o"(Å%În?e¦ÈH?•Æ?-×?€ö4†Ž´Â?î粑b=?–Ž'vâï?p<B6jz?sHE™E?ŸžÉ…ú¾?"Yfã3Í?îöÁž¬&?Š‰Tj	"?tÛö–æ?tò { ^?›öå1ïý"?†–cZø‡?í@ ¬rå%?ˆ–£Ë?É8ÁÞh?sí£ÇóÜ ?²EӃQ,
?ŒL&pÃf¼AGN4FGL J0024.4+4647?Ôì%|*6ÏÀ/¥Þ7X[âÀ:þŠBäÀ<`;`(^Ä@½$Ö¤@Œ…=Â?Ã4øŤ"¿«Á}ä1m?æÀPQ_@	ïùÜOv¶¿àhˆ•â¿éiáyð‡¿ëEM|Š•¿ÊÐԙI聿ïÝˍ1¬J?î'¢ PØ`AGNbcuB3 0021+464?ï÷ù# v¶?Fûñ.×0	?"5É9î?´¹µN2"?KŽ.ô°Éá?E'3±@j?ïۗóÒG?rÔXõI«?A¢wè%ÝD?Q}úUháš?oÿnbnÂ#?p+á´Ö½?d¿{?…>0ô0íG?VQãm:OŽ?WÔìSïL?Šê‡mg?…&ýäU?ïèÊ"ªc?NÛãºÄ4Ý?,#êR΃F?Iû:Xm?es¦úÚîû?MLßú¢ƒ-?ïïÒ¬›æ?ZFŒï£¤¨?0Ž)¹÷?&¤#?\7%'×ú¦?Xì½à =Ä?ïæ+(ÞØ?™Iy¥ñ1T?Tö?!R
?k5Ô»?œ?‰ç­MÖw›?˜¨EPc'?ï0Ž•b0?)ÐÖ>2?_®€tš1Ë?d‹+AÆ?˜F&6ã?Ž\M¥þ–n?ïªÔ!×|?pÅÑd'u?NÑ)tã¶?FZÛb?ƒ]äùE§?pa¶tôAGN4FGL J0024.7+0349¿ï75"ØR£ÀM0i@5z5À:ß[†8"ÅÀ<t{i,êD@Ç-õ±q@	þCg]Ý?ÈcŸŒ¢»?¼Ù©¿Š¯?òî^íÌ!@ê0ðã­d?Ä"SçÞ¡?ï–7D9ë´¿é yó$÷¿áß-WQ­¿æ¤õ8%á¿ïóÉü7ôcAGNfsrq3FGL J0024.4+0350GB6 J0024+0349?ïö‹mî_?H¾ñGA´?}o*ç°?æ<ÿ'ðe?QaRXÙg?G±ÚÄñÄ?ïðf(M1?e"[&@W?*K¤ŠOt??R)®øc:?[ê;¹¼¿,?blªI&{ö?ï•ZEs–?€Ê ú˜V?`+FߞDÔ?fåéd¦©?†ž­"Ñï?|1¼fX?ïí†-J2?D#Eð¥ýÜ?,ô%\'¨%?äJî?µ ?`ª£¢rn?C<¤6Pû8?ïðáeÏ×]?Püº"ì
?(…Ö¨6–?!ֱļÇt?[,y˜5Ù
?NñA·UÈ|?ïÎQP÷á›?~ú-Ô?>Ôí¡'α?SÉRî´.?vêËï?Þ?{"ŹEy?ï]†÷ç"ß?†?E´@ï?iÎ%;ʘ¬?r>žlV[R?'\a'
?ƒY×Ñ!Ã?ïÍ"ñ$?cÔ:T‹?CƒÇÓ}?4"Ÿ?wDýš°?c.wSŸíwAGN4FGL J0025.2-2231?ïåCûq>ËÀTŸ!BoçÀ;'›]:À<®ÑOŒÊ@u*ÑsP@#5ߵݝ?Âí'úÆ°(¿¢‹ìCíþ?ß¡J½éZ!@àë¡y6ù?ïÿÃF1=¿ásÁ}ä1m¿í§À8iÓÙ?°‡Ãs¢º¿ïÿØþ3w&?ïþ7ޓž®AGNfsrqPMN J0025-2228?ï½Sû{?ˆ5Y]|M}?Vè@
…×?`nzÖc»?{ÄFU˜¹?†qðÐe9?ïÊbÖ¨²€?'S²À?V@ýÈV"6?xµûµz™!?u>U!ƒ×?v͚Gs?í>æäóW?¤ p1ó'?'Ã6ýia?…Ð=hÂìa?³»€cn?£€2Îz?ïãþÅËÚ<?T|÷S´_$?CX#¸*ü?5ŠI Ë?g+1ä8}?RWÀ_nä?ï²Ù7®ü?ˆÈ6"Vã?aÃóªc?cìج6'?}±jO
öo?†¥¿ã*?ï{8UºzB?•e<+´d?`‹Á:WŸ»?w¨ç*t/k?ú4]+Š?'vŐ4Äl?ìØx7ÛIÎ?£ÝC
WÆ?"ÉþfLæ
?‡Êzòkk?¶¢þtÊK?¢ÕÁ
¸½?ïŸþ°t§r?y0	|e_5?d•OCR?dQG¨«Ê?'ÛZÀþ©?uJ\­È€-AGN4FGL J0025.7-4801?ëґTH#ÀQ!©æî·À:aŠ ÒHÀ<"P/Ã<*@H¹»øê?ÿm…/J?ÍiKH'áñ?Ê3E½#Œw?ÿ±¦Ö˜þ@I";ø¿çqCĐ¿Âw&gÈþ¿äZ1®
j¿ßýäqÚ
¿ë	^î¢àj¿ïÿÀ¿ù)ÍAGNbcuSUMSS J002545-480356?ï﾿Böu?V=)NS…C?AåEQT'?6F=MÊ?WÁ
œ?RՕÇs?ïð"ѪñÊ?f¾5kÚâ?*@è¤?=$Æ9»ºj?\r\@®(?d"z›ØQ?ï]"ߟÈ?ˆ"§S_B?rúzИø?wûéæ#8&?!Šá'N?"‰Þí_	=?ïó\)Å?:2À›º™?$[Ësòá?
ÆÑÌ/L?V¼GÝyï5?9Eiò ?ïåX{[ö?^•þ¬³DÃ?NŠ# "0÷?G.½þÕ¨?cû÷a'Ã?WC%¡œí?ïԆk$ÍP?zԉgÆÛk?6:ä…÷E?H³¯¤k?tYe¡Z?ys†É(­?ï _W9´?'/ÍyÐ8ƒ?y_²R2•?}ÌQí%?™d{\æ?šúƒ—´?ïäDX}"H?Vœ®¦üH?1
2syiË?#4"åf¸?išU)ò?V	zC
SúAGN4FGL J0026.6-4600¿È&	Ê.6õÀQžÏ€Ü3rÀ:Îùn‡QÀ<µG› @헗‹ÍS?þë׉¿1?Á!q)búÌ?†óxæ¤Aò?É»g_4Ã×@üe+Rê?ï÷´×ãD¿ã§E‰w§¿Þ€§ZL|°¿×ÂC[õIC¿æ›ëþì.½?®¬ù$AGNbll3FGL J0026.7-46031RXS J002636.3-460101?ïèl´;å?T²'(,'$?;2*IÄÙ?/OÙc˜à?d"Pÿؗ?R÷«i\?ïÙO{i`?s&@±v>?C™¦nÍ¥c?J…$ãÖPõ?på<àOi?pΧTWš?ï|ÿ€0ðk?wú¹°jŠp?b‹µÉܞ?iS_%æ~?Œ:=
ˆ›ô?sÒÂ_¬}?ﺋmˤH?YiY5ªtœ?H–á•iPú?-UæâD?§mÃPS?X²ªWo.?ïØqùº?aZpw)Õ?G§u×¹N?7§Frn?pÒ¹cL?_çKdh›†?ï" Áx}?‰"®ƒðí?O‡Ç.£?[W‰|´'4?ˆîß^YXŠ?‡^Ä[é?ï!fbñ£?ƒ:ÐQ¹Ë†?fdFq@™?h3²Ôg?™ª×(¥?€ýØ]Ñ£À?ï:õpLÿ?xh­‹7"è?^•z—ø?Il-¢^2?–·úVžM?xä¶!³AGN4FGL J0028.1+7505¿Ûø¹"ñké@(–G™ÅXÀ:Üéä4È_À<¶‡•@y56Ì?ü½3«(?ɯ_Éî?Û'‡W@
Ä_@wÏ@d
+' *¿åJ¬–Ì_À¿ê,9¿iaî¿­ª±ÄޖϿÚÛ5{Ù¿åøšá"¿ïÿGuܦAGNbcu3FGL J0028.6+7507GB6 J0028+7506?îz.9¤;‰?™ˆ8è¿?'ºFö$-3?‡šôn™"%?ÿñÎu)´?""7阍ë?íSX¶¿3 ?±åÌï¯ï?"'̃¾Ë?"€FŠž—?°[y•›œÏ?¯È–PF»ç?í/WO-uë?¡ÒåxfÚZ?¤úÐæí8?˜ÆX"k²V?¨º'ñ›?•3Xw.mx?íivO"ä?‡±ä,ÿD?"Ý|à_؁?s¶P
Î?®ùÜ¡nN?ƒàSÒ7e?ìÆn…*!?­wi¬·›?¢žLõ¶'?œ€4=«N{?°}eZ'h?¦]Î
$çÒ?é@tL-*0?Ã.æ–ç&"?­Ñe{Älb?±~\~ëtV?ÉÕp#Bi?À8։È!?êó~ŸÃ)`?©"dCöÂ?³#.Bï?£þþ¸­0$?µ@ÜÁ›ó?ûS?d'G?éH.àñ¥}?¢eŒ'gSÉ?¦¼¶Ù_F%?F[8rÓ«?Å0ÄηÅ?ŸÇñ¿ÍXAGN4FGL J0028.4+2001¿éè5fZPÀEAÑöy}À9‰þçÒÑÀ<B_•'Í@¹T
¬ç@Þ=½Ð°‡?±ÜæàÊ/º?¼l¡
ž¿@Ôøš°ðÎ@•wO>'?ïíKþSý¿áH€Âˆ%S¿ç{š—¿ãðgȖݿîÊˆNî{¿ÉxN…ÊðAGNfsrq3FGL J0028.8+1951TXS 0025+197?ïAædý?À%&'B1u?Püjè|=?x$ì"*~`?–¾Œ¦âš?¿gWt}wÇ?ï҆jgÒÍ?y4eü®©?F~V¢
Q?U´‰£Ø?súÛ½d?tøyí
"°?ï°ÂHB®?x1ȧ?dcR0¶˜Ž?ní²aBæ?}m2æå°Q?r	ç¼:¤?ï؜ßIQ-?Pkš´÷ðô?V‹âøai?;SŽ9‡?l\ڛ÷RÁ?JPâÒ¡u\?ï¥OòÓéï?§|š$@í?WÁ•ë?m"ãa9Ý?ƒ³ß¦{LÐ?¥³£ÛàÑ?k)2˜?Œl"kË?Vj"›ü?i‰oIHÒ7?‹áb¯Be?ˆ‡ùÖL&?ïsu#~Æk?'µôÚ
4¦?p:8Ãeyè?sXè¦Ön»?‹š¯ÕVo?~~bKn§I?ï‹Èë8?.?rþˆÀ³*ç?q@WOÞÂ?^)˜lë?"m¿‰·á?lM?¦™"_AGN4FGL J0028.8-0112¿ï46φ!ÀOÁàâiÀ;f؁5õ…À<œÉÄÐo@ 	{XæËü@ Ï[†I?ÏèEú
G­?wS¨ÀöLD?£É<quc@ù'#V?ïþž¹"¿èœ³sӌ¿é!P|ð§¿ÑÒ¸~âH¿â³'ÒÓø¿Üj¨ À€AGNbllPKS 0026-014?ïÓ	cšÈÝ?kŽÄ5D÷~?0C¢&½ýO?56lR£±?uw,\}M?jهO%?ïÀuÀÃÌj?['4æà¡?R{§ ]è?\"¹Û®g?{&5èOû7?z!:?Œø?ïF\°°?Š	PO'~6?aDODö¦þ?[Æ}C÷Íi?šNª‰¶4 ?‰Î)õ³%?ï'ÿÌZƒ?lÈ+‹r²?>Œ±·]–?$¶i"‰=j?Š‹Âç&Ýh?lcx0üj?סּ2ùA?{КÐ?>½5HÔo<?>­L•Ÿ
?ƒ©ÉI)?z|ñ"Ef?ï}­'"ª?'†ÕQ?Tôvg@þ?e7¤ú#[Ë?öÇ.Â?SoœM±—?îCRòã"A?"®3֔?i‹î§[‰?i\WN-{?ª2î;À?";r÷ã3¾?Bþ¾s?Œ®Ä߅œ?W³[Ù7óÆ?LRïÍ	?§) ï:•:?Œ°øqE†€AGN4FGL J0028.9+3553?‡É¹¬ewtÀ:ÁòfºI=À:…ðÍ]…À<x4Ô#&@Ržý0ÂÁ@"*ú?Àv\¨¢v?"ib''ž?ÅAÓ_
+¸@ô1ÿ¬s¿¶Là®V4¿âcK^£#†¿è𠬳R¿ÒýcÃHê¿ëGÝ^ëGâ¿ïÿÐÀL`×AGNbcuGB6 J0028+3550?'dÚ?ˆý`ܘV?Y†©²Øc;?Lm³['p?…) õ=æ2?};œ>á¦q?ïÞÁ€WB ?mÆi ù÷?;ZýR›-´?F/TÖt´Æ?mÓÒü7Y?i8ïƒ-¸õ?˜.›°?}"ïM‹Ë?cÈÐ7ë?l¢ö•Ã(8?‡!PM"?xùN^RˆÈ?ïÏoCYÇ?R[!ɇR¯?QF¼ÄkPB?3uœã_(§?t%?Æ,]?Pde-ùÝ?ï:ó1.~?òÓǒÑ(?l2©Ç+?_«ˆ™Á—?•³ƒãjl?Tˆ"C'?ïŸoÍÔoë?…ã);ªÔi?D;Ìw"[ç?Rm¸{mDã?†àO΃â÷?…»I‡ˆ?ï"ŸW§9s?ŠWÁ`qªž?kG‹íM±?o¬qÑ?˜C#Š+?‡Õ¥Mã©?ïÓ4…Ä?oø¬Èú?g•‹G:^ó?RG/@î³V?‰¥ØØxñf?kÅ$(ՔxAGN4FGL J0029.0-7044¿ä ÖWm­¶ÀG"—Oß;À9ñÇ9åÔÜÀ<|"ÿ‰;@jÆm¸@k›v¬?·»Z‰Ž^¨?¢ÿËÒ¦Ö?èfÓP0š@‰UC©M?ïÏ8''
¿æ_>ߎÆW¿âPÿÌÔY‰¿Û+ÝÿO+¿ë‹Ÿps/£¿äýÛb'ÆAGNbll3FGL J0029.1-7045PKS 0026-710?ïèË·ÆM?YÆnv½ö?BôB"A??8!)KØ?c64HŸ¿˜?UÂþ$†'?ïáìkpò?q7Fƒ*ì?<µœ¶{3?M¼'-ŒD?j|àñ/ú7?lÎ$a›gÛ?ïh‹€bw*?ŠÜ¹ë#?}ÈHÞ#i?…L8êa›?†øûràCã?"™|@×ÜV?ïÞ?›¡[°?QWé+ÃIa?KÙÎ0$M?0tˆúónu?jÉð—^Ù8?O|Ý	y¡?ï՗åB/?iVÞéW7?U§ôêã³?O%SW³¹?o" ]>†»?c˜PµÏV&?ï­5¤&»?†¶Ò>ś?F̝o?'?Yÿ1W:?ƒQ¨Â>ÿ?"D–rF¾0?ïY@ç.€z?Œá]·òô?y¾Z`,È?ƒcÔêÁ=?ŒÐ˜÷AÇI?"áh²"]?隣‰>F{?l‹4éL"ƒ?b»«ëA?OM´šë†k?dØMÅ?hԟR¸ØþAGN4FGL J0029.4+2051¿ïnŽ#LhíÀDÛG"#À;e‰˜š–À<¹"²²o@"töL"?öó•Þùõû?Ö"ˆô'?Óq"€¥×À@' ùà+N?ÿjDŒ¡äl¿ïß|7‰¿í8Ô'4!p?ìpéý_;Ð?ӎ˜ßŠi¦¿àXºvˆóY¿n(™) ÏAGNbcuNVSS J002928+205332?ï®9äÅ_?jEw
?D9'»"d?5
¢˜y­?ƒ-ô{°¯?
¥W1?ï—úŠA¯D?ŠÈæȨN?^çú&†ï?h›oTÈ‹?†$^½\!?…õ¤Ï†$B?î–Ó'7|?˜.l¹q.?x'ó q?ÿ'¦Ì).?£'ԏu±?•×¢Ä	?îH.ìÁM¬?¢¸(há?Sÿ,},íœ?Er™TÄ5?ªÝÍÅþÏ?z_ÜMb"?ï`ì;0¥?€Påy+?S6ªMÔCÄ?KR*™pí(?'¯VÔM?ŽK0à/›?ïîú§¯?–»¿Ÿ—Ô?f4Èüé?rÄ÷¡ý¸G?œ[‡‹In?"&ɧÛ$?í¸Hz†ó"?¡ÊT²ÀÏA?y/ß²Î?J^ષ?°ªÃNÔv?¡\r:;Ý?ë­kU'F?ªz€ßX?a°¥'ÙãŠ?`¸"\}"½?Áìx9?ª‰:Û
$AGN4FGL J0030.2-1647¿ãN¢»^îÖÀS¤5"_õÀ:YÚ´¢À<\ãW±˜@ ŠÞOV)'?úB`²È>É?ÁÚ­àùT•?Á+"V´l¯@—ãÓs@g[¢¾Š?ïÛÛÞb¡`¿½ˆGù黿À´±øàüÛ¿Òµ(kY¿Þ×e­ê¿ÖN²?­¿ìAGNbll3FGL J0030.2-16462MASS J00302045-1647130?ïô¡{ÿï~?GJ†´ê³o?#\iÊÀ&?uáS¾ó§?TLÜê3µn?F7ç»?ïæÓJY.^?lÅt¤¦Ã?2Ît€ƒ?E.KIëp2?fÒçg.—«?hnÜ´"ë=?´iØ?zÀÀàZñ?RmˆÆ™÷?V;ö§ñÞñ?…
!ÓCÇF?yÊÏë'é4?ïŒÖ
}'?f7 i^=Ð?B‹j@<?,,áa×a?‹¡Ï»B…?f¬V ç?ïîb/?RP	bÁI™?7ü"Ïǖ¯?/gƕd3?]Ø+	sê?PW&Ä\£¤?ﱉÃôÈ%?"ÉòÔ}®?FP¿—Û?STÕefÒî?'8'ùÕ#Ÿ?ƒO¼ïʪ?ïWvlÿîÉ?‰.ˆEâ¢?W8`Àk"?IkÁ, =?"¬Y×æ?‰lΠ¼˜?îäH=uE@?ørXH6?RŽø?'A?E"FŒÞ˜È?¡'c­r–?¯Oä›××AGN4FGL J0030.3-4224¿ïû}(8ÀR‡öý!ÿ.À8â'­ÄÊÀ<1˜F³B¸@¾èÈUï¡@å|Æúü?£Hl!ޙu?ªCŽJ0%@?ÞèXD@u9ÉOiË¿×&F{9‡5¿äúNEq¿ç3SÿÜn«¿æœ}ώž¿î":귙_?ÆNÖgUN¼AGNfsrq3FGL J0030.3-4223PKS 0027-426?ïåtYKÔG?iàAïo¬9?@ž[نn?>	"Gµ??fd@5oæ?gŸŒX"?ïîýë?Šq©®HÓ?SÔH–m§e?omڀ–÷©?y{–|kNð?…†éh¹ÒÊ?¶oúJ?›ª¸]ü?w#ÀÒ(8|?õrì²I'?¢Q¬}ÉoÐ?š¶'퐹7?ïè¾wõZ
?MbKÃï0q?Lþ¸$o±?8ÃÄf6¨^?`Ú
8µò?GzÖ¢âP?ï²Æ;ìÖ?''4n'Fù?Vd{Ã?h*;P*À>?€Ždg¡º{?õø,ê?ï_6ÁÞ[?¬¿Øa¤þ?u|ØúT0?¥•ðL?tK"àw?˜S¶ªYVõ?îñ'äºC?£89U¬ÇÙ?tՔ:ïÉ?|«ÙsŽ\?­&:÷(¿2?¢Þ—)Æ°¦?ﹿQ9-ž?qÐI)üÀ?gÏ-Æ&s?[›´¹!7?w8Àž'¾
?kµ‹Ý*RcAGN4FGL J0030.6-0212¿æ"õ»áöˆÀP%‹'¢À8Éõª;¨MÀ;ã{ÕctD@—ä´,@e…—"?§$ñž_Éa?Àpü}êg@°y=Ùc@XÕ
¥?²р)ŸÐ¿àZÖk­Î¿æ¯Ãzm"¿äqêÉ7¿ì"C çU¿ïÿ%¯¼ñAGNbcu3FGL J0030.7-0209PKS B0027-024?ï´f¸´?'ËžÜ"?q&ÿ¾|«	?'M­¯g?tÎMJt?gu<3·8x?ïévš'?pÿ›PZæ?3±Yϋ5V?NS'ì6•_?dS8ö?jk§Á«Þ?ï@ä\ò…?'›)®Ó|9?y+ø>[(œ?ƒLE.܂?'˜vK9Mú?ŠbÁš=?ïõ†	?<;7=s"?%ǁ½\Ë?ãÀ8ÿ¢Ð?R:ä?9'/b!ìè?ï\çWù¢T?ˆþ_y´¸3?w‡3Ýrwo?oÐ	wå?`\?"ÅiãÝ­?ïÇ9eû?R"
>¢•?IrQ	ƒ?cgczÇq?y5.à9"x?|m²è}Ñ?ï'ô­*^è?•fûþà¾?yfɀ™šÕ?'Ë8̜ö?"§¸tÖ??"4ÄÖÿê?ïå(Á?O÷?Zv?5¬?<˜ÎÎÚRµ?2³k£¡Š?gD$æ÷íÎ?Xú|©AGN4FGL J0031.3+0726?Ýtª7eÀKŠýq?À:è7Åi+=À<•(+˜4?@ €³¾"æ?ý\\ø(›*?Ç/–Æ€'q?¶/O"ýÛã?ðœcÈý4t@…¼¿äqN õC¿ìàß8³¦?ãE—Ne¾¡¿èüᛐë?™<ä"Eí¿ãÕàòž™AGNbll3FGL J0031.3+0724NVSS J003119+072456?ï™!['Ä?­tÃØ·†?1>''–W?!ÚŸ/ß?‰-µ8›8?­u^ Ó§`?ïÑÎÏ4¨?t}=nÓ¤?D´à¦*B?NàÐ[,Në?t'b£"ÁW?qSaª«–ò?ï"Sàì?‡C
Uëÿ?[¸t
ËÙZ?Gkåk—}¤?™ònSþ?‡‹=²Ô?ï›_GcA?k6C‰CÂl?*Éᅲbc?"~r‡,ƒ'?ˆÎÀlí>?kIsVXæ?ï;Æû;?'¬¤ŸmTR?D™JX¯?;Ñ­úOÃ?—ârØ8˜?'"¸p{;€?ïˆAa8?ŒQ,B~)Ò?M9P´MV×?^‰ã¶KÁ?Œ˜#›è?Š[JÜû¡ª?îPxU¶?"îj>RÅ!?c,îß¿î@?_/r¾I`v?©Å«¾†ÏB?"Ô†Õq¶ý?îë'#È÷?ˆ"+ރ˜ ?;š/½-/?<b£8Å=?¡ª¾–9y?ˆy¬"H!AGN4FGL J0032.3-5522?ç!¢œÍ€§ÀNÆE܃#6À:MŽz¦^À<|R¢dCv@(W·L@ó•$Ý?¹JÔ»?Ś"U•]Ë@	Ëþp³Ç@¶|‰"g¿Ç
G_ɔ¿ÔÍ×ú'xë¿ä¯JÛÆdÔ¿æ+|_÷âO¿âVlSq¿ïÿòÿf}
AGNbcu3FGL J0032.3-5522SUMSS J003210-552228?ïnœÀÀ?²Ò&
Ó.?Q98ìÔ3?}	Êo'"?Š"ýe€iE?²@ÌçKi?ïôm9-7
?`$³]?$€ÓLû˜?:²pyëw?T£©ñ™ø?\FÅVIÚ]?ïŒ;­Þ¨ ?"]°M"è?k~xL$?s<E5«;å?†m5™‡)? Œå%â?ïü&‹¥? "Þ݉zö>ü7>Z²&ø>è7Öæü'^?='¦? cƒ)ž¦?ïåYŸó>À?_ݲ̾-¦?Nìþ'ÐY¥?Dª¶¤Û"?bë Tö/Ô?Z9ñÐÖ´e?ï×ô.ö?{¥i#@]?6âèF•°•?J½ðr™?sWií?zŠÝñç©?ï:_ƒ."^?‹ºÇ^^ó?yË 'ˆU?|pÊĽ?'AGyåiê?†é¤Ô>£?ïöŽ¾y«?@S×ènyœ?ùǘè?ë*¨dβ?QÔkÆÝRŒ??aâĕü˜AGN4FGL J0032.4-2849¿í6S›ðÀU^c^J8À:ã¹L½GõÀ<¿×ç³ @»ï¶ÝÍ@mnÛí÷?Äy™ßd©ù?·JÌå¤?îè³³ S]@-½@gÏ¿åÜȝ¾|¿Ñø%?–¿åÔdcP¿æ#JóCY¿é¥va†,Õ¿µËÍô?,'AGNbll3FGL J0032.3-2852PMN J0032-2849?ﻢo£sZ?pÓdãÓÓ?K¤GÍ:°??è]n2ÂQ?~ºDýe'ï?o¯òG?ïÃû¹/8?}}u°'ü?JJŽ‰«‹]?Q¤fÖë‹?z¸Ñ{í¥?zÆ.Bˑ?ï2&D|¥?‹ÃÉ0ª?h˜†
¦æ?c^÷D52>?–¨&±6òš?‹
éÐÚÂ?ïÐÕ0.Ø?UCßDròx?GüdtÂ?0³9¦XJ?töˆ¼ãYÜ?Sí×rlÕ?ï;+r¨Æ?‹
@¸àdb?`Ï®>òM?Rcövø°…?–€›é!Ž'?‰íL…OñÁ?ïfR°Y­#?—ñĽ?\§¤"Ši?pƒÑ鑳'?'lŸz)÷?•ÃÓow]å?îuŽÒÁ-‡?•}s>¢8?y˜è¿Õ—?t«Kd®³Ž?¥sõ½~G¦?"^»+¢‹ª?ïo7Û0	U?wýœ¶þ.?_í&EyZÚ?Pd#T¾=?20SÚÉ?vß1.4üAGN4FGL J0033.3-2040?½XDq–g­ÀT•zxl"hÀ;ʦ—®ÞÀ<æMú^Ö@!?Ô¶P3Ÿ?ûØdàTi?υ˜…ÈVp?µ·@Hšx'?åD¸aý–?ø‹
ë@€N?Ç#v|´¬¿ïþµbLü2?ï˟`Xy¿ÄðáxÚ¿ë_÷auæ·¿x'Úì'ä~AGNbllRBS 0075?ï¹pÆôy?ƒwÆPªê?@¨iŒ$×Ì?3ú¥é}z?€™s§j.F?ƒQjI€—·?ï®v¶ü½?†ÅÓÚO?Z›/Šøè?dÝwQ‰¢8?ì]0À?'K{ÓYà?îÖbo-VÈ?"t—ßuÃ?rV%Ü?z½T}'R? Oxê?"~Ž•wÏ?¨'þ?†ä®—Œáì?\>W¡£
—?PÇëSC?¤³²¼®±)?†o¯#?ïtÕT…¾E?‰§Âê/e?Nh™oO9?Aöá}Cܨ?r¦†á?‰Vµ'ÿu?ïLQ_C1ƒ?™Œ"—d·?gvþJÎN?{))¬.?"‡±Í$Þ?–'.Îòj?îg1͂L?—#I…4Q?pقï,³?w ÎÈ`¾?§q²ã¬2/?–O#IsK?ì£O*_¥?£Ü²x+Ã?iœ SOçÙ?jÐÖzS5æ?º¥¨Æˆ:?£=rQAGN4FGL J0033.5-1921?ïð[DÐïÀTMäÍt'yÀ8<Sz
ˆÀ;Pv'¤‰¸@p0ÙÒá?ùꍺß?¢•¾î'Å??²‹À"¦£@|¿ôw5Â@:ÁmH,ê?ãC0×?³´¬š}DN¿ÙՐàãZ-¿Ô!&€È<o¿ÝŒ=ZÔaí¿ÝV"Š‹ßAGNbll3FGL J0033.6-1921KUV 00311-1938?ï²Ötžëò?'Â[2ž?`vP¨/Òµ?sq²·-Al?~YC´î?‹·Ÿn8Ð~?ï¹íTµAž?'ñÌguzÃ?OŒoúÊTÀ?gæá/É?Ç´?{V?º@—?ï-*c3‰£?"GÁËìò?y22˺ï!?ƒ5(·tm?"&î³$Ñ?€hLü8?ïbk©¶?"º™gœPÁ?YD‡•÷?D]œÿP?žCN*Ò³ä?"…
GTô?ï²ÿ/ºF§?ƒŠŸÎ`y~?T;D7´?_9˜Ý›ùß?€¼Œ›ØÛÈ?€Ïí¨Œi?ï€%¸²tÃ?™'"œ_Ü.?\á˜7ü?sñI…7hs?ŒZ^×b
L?˜;öjçF?ï
!èhé?—‡7Ï÷?{§ŽÛ݄?"_ò@"/Ö?—rŸï(?"k됦8¶?îG8ò¡?™ƒEhk®?c$öS?VÜZ®×)V?ª\^ƒK­?™‹ œ¾ÆAGN4FGL J0033.9+3858?ïè³æªwÀ7ÆÛ3—ÝÀ:h9Y½áwÀ<v[€YW@>|›Üë@Q«›úœê?Àj˜^D?©þñÀª³%?æíb6V@
¿Î÷õD?ïü¼ž×F"¿ãÆC{Ó¿å+$ p¸Ð¿çÕ)ÈPfJ¿åŽmìl¥¿èޝ´K!AGNbcuMG3 J003408+3901?ïïdr#¯?vKSßÕ?V5ö:f#½?v˜öÂ¥½¥?FK´éù?5ôªOU;1?ïçrßè?h&™złþ?1‰äò!p|?=npßÌ'?f[äs"Ìv?eÉ)tۃ¦?ïºÚ/ûŠ?e8Zés_=?T›µ('?AO•Þè¤À?}kú¹"í«?c«ž§¿ù?ïß^Û`A?I+Íï)¾?ITèZ;Ñj?*7…7t®®?jKêÄlq'?F…AŸØGx?ïîeDl/?Z"™¨Ç¯¹?AŽX#1?R´½å_l?[8	Àëç?P܎Ç:µ?ï­1ȋ0?" -F/g?Fµ€¿lN8?VôlÄéok?ƒQÛzq®—?'蘖×?ïŠ÷÷=]?v£!T¦Üá?aT(žFÆ?SÆ`'¼ÕS?ˆìø! tæ?t©!ªÕ@6?ï¥× Ãâ÷?hiÞý@ç?`â©ÈÛU?IL´Û?'QmXx?eðP‹æÚAGN4FGL J0034.0-4116¿ÑOɹ>rÀRÚu%F
¦À:}à{Ö:À<|Ïç/O@èOiõ'@"s9³õ?»ö•Žòø?"p?Ùð??Õò,'¿ãZ@‡æ¦'¦`?åÉTb,ðÏ¿åyêPì¿é'Ò§®/¿çD-÷Š¹¿ßg49eý¿ÜÙü€n¥OAGNbcuPKS 0031-415?ïùzB™á?9‡eGd?"(…öõ£Y?iŽ¦ç?EŒÓ'gF€?6f@§äMÿ?ïç‹J݅?i—eœšà?1ÚÍR':"?@õdÕD?f9[xo%?g!b_ÍnS?ï¹õt‹Ã?n=+¾L'á?S^T¶Èú?Fhj¹J3C?~?®@m¡û?lÎ<Ó3Ýí?ïô8~+<?6÷¨js¨ë?×gpßÛ?ê,Ü2`?UьÞÍæµ?6[kÒ1&?ïìêa]=?u	!ÞÂX®?4tdÍ}Uz?%Ý&þ­eR?`‡ó°k?tÿ÷"°?ï½^>hŠG?…ìöê«Ñ?@õ¾9g+Ç?T߂D²ôI?2(æºôÝ?ƒ"7xæ§?ç—\?x¸û_¸?]li¨—»¬?Z¸†!uN>?‰¦xíU.?v˅|d«)?ïÙ²ÝɆ?[©Ì=ã•?8eZqD~?)ìﰚû?qöMÑþe¥?Z»'XYÑAGN4FGL J0035.0-5728?ê˜(ÒuòåÀMÂDú<À:Ö-Ç©­À<—üñý@™ƒlÜw:@={ 1ί?Æ¢*cÖ¿?²PßkŠè|?é5Ü@W@"½a4?ïèËùo˜¿åªqѺ¨¿èMŒæ,ð#¿æ×ÔÓ+‹Ÿ¿ïþÓ°Üá?èÁ'e±ÍAGNbcuPMN J0035-5726?ïé(?XJT}i8?BŠUþNµŽ?5k ¨`?bU_`îAd?U¥­aj-¼?ï¼î9r×'?€¾éÞÎ&?VKaûË?`>è&Ô,ù?|]ÏͶ?z>{mµ?ïo†ê¯$µ?v×Ϧ–?kƁͫµ?içÎB8?]"¼²cÅ?ræç×rt?ïÎÏ}Eõ?WÃè€:*§?W˜Ûš¤=X?@°ë˜!ï?r²
…ë>?S©iò•9à?ï×Ø^{`t?hÞz…zh?Oq"LµÖØ?F'äK–:
?p%žL•/¬?fÈy«ú?ïW£	ÚÊ;?"ñ<M 4Í?g"$9¦?w.{ƒ<H?'*:…×X?'›"L?ï}Ý?O?‡œ.r¤Ð>?tE•±ô±?t€9þ«Ð?š^ßmÑØ?ƒÇ?ùKý ?ï\nbß\?ybÖrÀ¢T?rè<‰…Ç?aÍ[{›h¼?pIŒ‡r?t½NLb²éAGN4FGL J0035.2+1514¿ãŒ7ÐjªÝÀG¹‰a=1ºÀ90õ üÐÀ;¾mÏç3€@Jz'ýö»?û{fX#­"?®Œæ>.û?´Àû³?2@	QÁ
{é…@
ë±îO(‡?ÚqžÞ|øy¿Ø‹MÜ+åa¿Ù8PϞ¹¿Ø(.½'¬î¿ßqÂeؿṈý•¨AGNbll3FGL J0035.2+1513RX J0035.2+1515?ïõ÷6
†Ÿ?@œì@1d^?"^¡v?|paªîÞ?QÅÓ'¿•Œ?>‰ÞÎÿÏ?ï×›GĐ?r?OÓªE?Aÿð'yOç?J†ÈfíÐ?r543F%?pøÃ÷?U?ïªÁÔÈ£?v݋íò2?ZKÈQÿ+?W=R*þ?ÿ¡Mԇt?uGí3E,?îÅeghg?Œ{°›Úå?^³ÏŠHA-?@œu¡¬µ?¢´C‡?TÀ¥
â?ïê½F$°?RŒ"—'M?3Lé²jÔã?%áÐÉEÉ?bÙyýÙÊ?Q@Ëo¨ ?ï€!îÔ?Ž•7ę?U™H'ðR?ca}TÞ¹g?D[Z¶Þ8?ŒEmÒ©K7?ïŽ~0?O$­jÑ?aZÿª@˜
?eÿ"Mlä?ˆ	³ÕQx?~ÄÏpŸ´?ía2 ê?– #u Í?l²ù0l?V¯çr@=v?´Þa–T?–
n?³%/AGN4FGL J0035.8-0837¿â;"ãæދÀQÈéᰉ À;[ø–2æÀ<´"Š‹ß@+2w÷]o?ÿ˜òtý?Óâ?»+åŒ?Їç^j?úEû7Cc@Ó³#Ñ¿ïý?üoQÇ?î|r!/¥Š¿Ý"m?ž{¿Ö3ªýD8ê¿å÷C~Ý¿ïüRáÏ=jAGNbllPMN J0035-0836?ïê­íõ£?Ra8ì½þ]??¨•y`?.º@D°?bœ×¿X?P_ùÛ>?ïÛûBÎS,?q f‡€í?@)XÕÑÁ?Hb cœ¨?oúg¯5?ný…BD×?¥¾ý?~αgbX?c7î8?g^Õø>pv?‰ÉÐC#ì?z_GÚu?8RØ?gpÁ"e€Æ?T–ˆvÀS?;É°Í?ˆ'(gà?fqÄÉ@?ïÑrÑÁ~?fa¾A&?PK'äl?B;–ÁÆ8Ý?sB봄ܒ?c•ÇûsR¯??¼¥Û?Œ 6	ßú<?TV¤ƒ?cû~á¥?‰%KÊöâ?ŠP±Â\Þ?ïC؎ï>?"H;×Fû?gŽ¥ g,?dç?¼Cíµ?"¡ÜKTn?ƒ(ACD;?î÷ä^~2?'¸™Äù¢û?b],Vü5M?UF÷ÑTfJ?ž·×ã¥X?'+gl2É¥AGN4FGL J0035.8+6131¿ÀÖÀ…ZŒ¿ô­6À9«½¿é{À;ZÿÁße@gˆGa¾a@
{ 1ί?ÇxÐvO'?¼Š"AeÐê?ô¶Ë8x'@
(ùÿ
È?ïÿǀ²—í¿àJú¿ú+€¿è—Z$8Ä¿äöö6R¢d¿ïúú!™­¼¿ë²u"–ØÊAGNbcuLQAC 008+061	?ï€NÂ/åÌ?ùƒÉ€?@Êè1‡U'?A¯©7ès?Žß áwÙÊ?hl°?hð?èI-å°7?ÂéÞSe‹S?sاhe¢M?yÜìYÎá!?Î=
ƒ‡p?¨sž©Ñ?íŽó<<
?Ÿ:b¤ÿå?…°¾ç@r?€^-ÐMUã?´r²O‹?ºiÈƂÜ?ììULÒZo?Œ¿Ýº«™?‡DEev³?dÊ2?w¢?µ´Ì꘩s?‹@uãrZÚ?îPˆ·&Ñ?¦û·˜sƒú?QM_{
/?NxïXoM?®ŒzƒF?¦ÆÞÊ«S?á+1WÍ·?ȇ²—Ó'?"VkRN£q?–‡|G?ÝéõbÔG?ÈcÈd»Éù?ê`('Mþ?¬•˜Ò (?"q´AHqI?‹>±QØK?Ã\HÖ2§?ªfjŸßm‰?èABÈ:ä?£	ðzÄß?Çž¥ø´?'–³âÐW6?ËBÐÄþø?¢ý%F˜AGN4FGL J0035.9+5950¿Ÿw)Òö<ÀÖCEÏíéÀ7ñûš°À;B¬ï¡
@ $|ÍÛëy?ú•†_*2? bGÎ\š?ª¸Å-ò@
ø¤™§ÜR@'"ŽJ[?ï° F\¿Á.ÃâÃY1¿Ý­êžïÄÉ¿ÑÓ
X®ÿ¿ÛB?•—,¿Öîï!
'©AGNbll3FGL J0035.9+59491ES 0033+595?ïʷՀ
ã?j
ÎLÃô?0Š×ÀããÔ?"˜¢SOü?y›g¶ÝÌ?i~ª¡œüß?îºlð:²?³"ÜÍI??Iš*<Àêl?_¹Ž'/Ð?­­ð‡ŸÃ–?²ð¤KoO?îª	zQï?—^1^}Öô?jàÝ~†I?s''20@E?£±aÝ Ê(?–=eç
C?ï–N®cÖ?jŽYna)·?Iç6ª/?13§jí?ˆÍàþEg?iú
ma?ïöŸ{}F?Bj´,›?=.Œ½`›¾?2¿ú¹â¸?ŠØã³""›?€ù§"ݸò?ê¾ðЯ|Ò?ÅG–†ó,?bëåbŽJ?‡ãÆ3až"?ĸ)­|?Å*'BëÀ‹?íþÿ	ûN? D4}¨·?r;äA?wã5½NÇ
?­È®¼Ü?ŸrxS´ï?ï#'º"à?"ëb:çðZ?YÕ܍®'¡?Hî=Rßó?™ýªëD"×?"''š²DøAGN4FGL J0036.9+1832?ÔzBWN¬ÀFÝ/Ÿ¾À:Yºû1À<n}îBh@g*&š£@'L©%þ—?ÀCW÷ã§?¼Ìõ''5?ûz&6Ën@ªk­Î¿æÚ³ì+¿àú®/«¿æ,@Ъ¨¿çÞ¯°î¿×)9_G8N¿ïÿÁìžú,AGNbcuCRATES J003659.39+183203.7?ïñ#k"ùw?SÄkWy}?#=K×´•¸?Ï{ql'?[QͶCÙ?SÏ%Ês?ïìø¦ÅQ-?e³ÈŽ‹ˆß?*â@ýÆj?:¿±Ÿ¥à³?aeû1ÁX?c~,²˜¡?蓼½w±?x‹V­5Ù?R¨%…ðú9?;–G§ÎÙt?ƒÊKâ-f}?xEÅêTüí?ïøà†4"c?.ýÍÄÄ?q}q{w>óÃëGƲ¢?KÖvfñ±?.Ö߀¿â?ïß÷ªy™R?eSc0OHÖ?5¿Hۚ»T?/\àÎZð'?mPl¢EÓ?d×á÷Øô?ïÆ\Âg‡è?ûf o?7×uiG]x?L" Gns?{T'd¿èy?~rË/
?ïS-zü9?‡Cü8ˆ"G?a…3s8?a'ð:èê?"nÓôé‰b?…Ò'"?ïì?ð'?O×%‹Ü,V?  nã˜M…?-KÜôˆ?bíæ
¶ ?On÷WAGN4FGL J0037.6+3653?ì`Ÿ"ŒŽ'À9ä—{žÀ:ÌÿؒӭÀ<t1rhÓ(@ÆXIî@$UšfH3?ÉÌS•©J?»zàÆÔ».?ðÇ#Zx›@Dt€ª_¿í¾ûˆ¡ú'¿ºÕ¢"C¿åÑÁD®[¿ØkYë-àä¿ìmˆcç0%¿ïÿÃßé47AGNfsrq4C +36.01?9YVÍ?ˆžÁ'*;G?Zú;˜yz?[OЩüjV?ˆ*:b½À?…É®Û~?ïÎThPæ?sRÍä™,?HÛØþfQ^?T‡-¼ìÑð?uºPΣ‰?pžk²þ|?ï?–¦Óœ}?…høݎöY?r'•èP^,?r¿3¨I)?"l…±§¤Â?ƒ
všsÛ°?iìáH?dtN)°\ç?g9׊ã™?G~çCŽk?‡‹ïÃäõ!?b Öê$þê?ï 'õai?0'Ò§˜?k[Á¹Ÿ¦ª?b:{Síƒ?˜‰0¦ø
?Šö )×o?ïZ&•d?'ăçí?a,˜²¼qà?s^¨žÆ‡j?'ˆÈ(1Ô7?Ü>Üi	õ?î¿'×$-?'¦N;æs?v–ÿDõü'?vÃ"¤4?¡;gçÉ<?æa´«ë?îÞá<Îðò?'g'sg?zð
~Ω$?d"zýlêÉ?gÕ}{?€¥Z°¹:†AGN4FGL J0037.8+1239¿¢®X½bIíÀI
¥¤i×4À9€C`§à"À<+»Ù_'G@¶I'uç@ÁªYÛ=©?­²ÿµò¿rÔåþªä?ÃÓ·79R1@z~ædùT?ïÆZAêÜ¿â咖pn¿ä›:]ôÒпà+Ôßë¸u¿ãÏß Œg'¿ã]åÄ—gAGNbll3FGL J0037.9+1239NVSS J003750+123818?ïêÃ$`?€@SWïï?+Jãð× i?5À›Á«>|?d:Ži¸G?˕býÏ?ïî +ïr?f‰ó¿
r?+Ð\ä‰?=€Ð.ÖÑ?`"ÓÏSo~?d0]í=?ﻹp"TË?p¶Eˆ®§?R—Rßü?<!áRŒv€?}¡@om^p?p;i?æ<?ïîzÔ\Ž?@s#ÁÑîV?04x6¿ã¢?@éÁä‰s?_ïì/ÀAa?>˜å+q?ï͇D­Y?‡»òê*Ç"?@Ñ(ú´Ú'?I–Å-,:i?w"8}ä¡?†YžÞ¦3É?ï¶FV.>?'/ӛ]À?<¤À±L?PbÓWÊa?|ڐÄXÀÿ?-[V╯?ï'C‰Æ?wۉðÛ}?[yrÞHe?Pȸ7Ÿ?ˆ@ªÙ»{?vXñý>ŸÅ?ïÔâòöNž?\"ÔkÌ´©?E"™+Ý?2¹A|çz*?rêD†´ô?ZAž{ð­"AGN4FGL J0037.9+2612?ï6›gÏòòÀBI/Ÿ¾wÀ:×Dœè³À<ˆ')ó@+QّG@ì楻æË?Ì.sEqú?Ã'À²7J?óŒÙ|Þwð?û҃Ee¿Û@`óJ:¿à'È>Ȓ«¿ä¡wÿ•÷Ï¿è"J½¾g¿é.†%HŽå¿ðAGNbllWISE J003719.15+261312.6?ï¹{.ÓÓ?…2Rïƒ^ƒ?Q^Y]±?]%Ïu†-n?Pãù^X?ëþotë"?ïhԎÑÙ@?‡?Þӏ¨?kIiy@È?kDä-¸I?Žøñ@?ƒSh)V‡î?ï-NCý'U?†±F¾Ý?x˜ïãmÇ0?x{™²¥Ð{?"/û†£¼–?'cRPªöb?îö'§Q'?u•îù¤DŽ?€h<öE?`r%"Çl?™#4öGh¡?r)bP·ex?ï(xœ@_c?ŽÞä+­À?fÆïëÆD@?^ÊQH Bÿ?˜ƒjG
?™…µ|6?î2w'S½þ?¤D"pwŸ9?€Á8GƒÈ?ƒBÚew?¨ØWŽ&'?¢gf‹b9Õ?îHŽŠ?"‡Ú2µ?…ž@E¶Ä?"©2ëoC?¢£ïâ:B'?Œë£|œ]Ä?íqÂ2$O?'±×›}?¦Þ¾¡AØ?|páÔÍd?°H6Án[?1<pO—AGN4FGL J0038.1+0012¿ëýò,5p®ÀO<±î$5iÀ:úûö†À<_zù›añ@»…øÒå@
¥|üªá?¶	Ê?eò?–õxί?âp¢qON@ï72œ4¿ç•¿x¿ØCûlóHb¿åCW}ÀJ2¿Óîᵒ¿âvOb=⺿â˜H+ü'AGNbll3FGL J0038.0+0012NVSS J003808+001336?ïÂÕú6×?j~ðˆ.³?L+è¡l×|?<ċbOõ¿?{…¸ŸñÞ?h+œÈ™}'?ïÖÊ42?tëø:©""?AÅE÷†O?Mkm'Ûs6?rbC{Þ¨V?rWîä~ä?ïjjèxœ?}°¸ý´Œ"?g¨üî:¡5?cÕÓzh_?¦YҒ?yTƒö©Cø?ïYÖŽV?p숇?bŒR/Œ'?Gqã'Ø¿5?'sµ«ßF–?nÛÕýÌ?ïƒUÇ]?}}Q1ô`d?`¢%ºû?Q	.wã1?‹©=/?zØG˜²¡M?fðØx? Ö<Ì´Û?WM­ö†y=?cñ+ØG>?Œ®0u*ÞØ?Œ×y@N?îëL©É4?Šcµ#fK3?s'öZ	?pÉëLèܐ?¸/*Ô÷?‡…ãæ6-Î?î[êý[Ø?Œ$u긧?xcx€[c`?fA2»ÓN?§CA~®?‰ô¢ÐAGN4FGL J0038.2-2459?ÞúÔaì""ÀU–Y_í¦aÀ8ùþz¾ãÀ;ùž$BÕh@8ÃäpØZ@Q¥Ãsˆ?¦e¯¡º?¶ÎQ ï¿@aƎÅ*A@žÌíY	\¿³ÍlÚɺŸ¿Û-+|…Œœ¿äï4 #b¿âˆõý¥¿ê@N¤©¿åó4«wªAGNfsrq3FGL J0038.0-2501PKS 0035-252?ïäöH`ç?\Á‹J«[?F?¦)é5?;üõ­1?eyÎã,›?Xœ[Ã?ïÞø.¶‡ø?…ÆKûÌ­?-}×í6)?JWŽ˜¤¥é?o/ó›Â5"?…B4þ›n3?ï"&á@LK?˜Jbì⫁?rš9"¦$?|µÆÊ¥»?—•Š×?—|VŠÆW?ïþ'W0—?§~/Òp>áè21äœ1>Ó¨ÁGw?%¼¤1g5?•0à/\?ïÉ,M©r?l¡=?M]ðùþ¨½?Bɵcmfš?w¾B@¬?iæF
E°?ï§ÈÒùÉ?—À®!	;È?FÝÎ,ŒˆÚ?g¼£½'­?"Ÿî'Pqs?—ˆ$÷è ¿?îòÐ/`sf?—©Yp­¾Ê?v‹â|ê4?}Ngœp?œš½c¬?–a
Í\–c?ïüä9¥é?+F{†&~Ô>ôFŸ?è>ð]]¬›£Š?7™Ò]û3?*n.LÍÆAGN4FGL J0038.7-0204¿ç[w4àÕÀP0¬![š[À: ñ68¡1À<F"—u@Ëßèˆj@÷ÇÀ?Åd¦¹
þ?̟6çrÀg@öÇd­ÿ'@óœÚ
οËB#;"Ü¿æBM'iÒ,¿ëÍQŒºŽ¿ï݄?•AE¿ïž©£Ò؀?Áþ0\"*šAGNrdg3C 17?ï½vh<)|?¶9ºÅ9	?T•Ž7à?Tª+™Ø?|"*u¸'?Ùu'T\?ït+Þ;p?'"€kzkd?t{v¶p5?'HèZ~?ˆžù¥©åp?‡&PÊä8?ï
ÛÛTòB?Þ#b	ÿ?v¢²ŒÏš©?s )hG©Å?˜û×ô•‹?Œk€aãk?ïo}|`+l?oÏTbÂÚ?t©,{Šm?YäþU³¡:?ŠLP¯}®?il£°^ƒ?ï'|E›?‡=܋Zt?c3¸$°J?bËú§Áôƒ?†")ÿ>\?"ä"yväc?îr>ç5H?ª6±çP_?‰lXŸ§›R?—Äå?ïÍ?¢"5åWA·?£ò$ˆìm?í×âLaë?^6žÚ"?‹Î‹KŸ¦ÿ?‡zÙ(ê?«Ž8m}އ?˜³JøªT?îµ=3£?'Ã
9ƒ5?ŸÒfìRŒ?X§Ÿ‹]?¦DŶœ…?÷F÷IóËAGN4FGL J0039.0-0946?î9{"Ôk…ÀR,ºËCÀ:#ª–A…À<f=°d·:@é3þà\@u{­ˆ?½í'þŘP?¹PXÝç§?öüºÑ!Æ@û!'ÌËË?ïÿmh¹&þ¿ãšQ_™¿¿é5Ù L£¿ètSß{%:¿ïÿñ_{'?í(#ÕÈAGNfsrq3FGL J0039.1-0939TXS 0036-099?ïߛ94‡¥?w€¨IUe?JXµ%lë?Yêxè÷¶=?iá0¯éÈÌ?uC7Ä.Æü?ï´Ê[#?€»ØíÇ55?\Öç54fx?dِ©?~e|ÞUì?z]õ?cîi?ïcØ©=ÀD?†¨ºH棹?pCÿ×6ÃA?u¼ÌîÀp~?ŽçÕÔµq?ƒ<tË?ïςEƒÜˆ?XgœÀlK–?^±agF0Ì?HªÅ¹‹Jµ?p'…lûÄ?Qq#º_ƒé?ïÏ?¾åa!?ró¹±v4?V•å³
Gn?]œ µÍ¢?rº§?yYŠ?m×W••4y?ï.žÿ4(&?ö%øÔ9?rÙZØöG?~䑬f®?•«é¼íg¿?™Hh}­?îß®Þ5?'e"Å©žÉ?|jx­²s?}tʗ'R-?œï†$á#?Ž«îû?ïgu¼€à?ycC~ª^õ?yu©,7Ú?keðÍm"?‰"œÁÉî?r2™±êfAGN4FGL J0039.1-2219¿ã?uù×FùÀUg8}¿À:…®Ús~}À<o­é¿@ ÚÒZ*mè?ü(—ξ??½
díj| ?sUÙë9I?¶©={‹'™?ÿ–ãìÎõÇ?ïàYÜë(¿Ö8è^£¤_¿Ôb·ðœµ®¿Õ1fªY~¿ãZ7ÿuÁx¿ÅíQ½ƒAGNbcu3FGL J0039.0-2218PMN J0039-2220?ïÄ`ÂW?m-ƒo+t?@½i)±~k?.AàÈFÉ?{·ñÙ)²?lPßK>"©?ï­ ¥8?Å:Z…©?Rb?àÑÈ?Z³ê»'?'n÷¡cÜ?×sEE?ïNMFk—?"Ò£oi?cvpÀ¡Œ'?eÀ;¦ ¾?"lj;'›?"WìN¿û?î·â?ìÆÅ%Sl?dXüѐÄ?JáI»¥"Õ?£<]ÃônÏ?~õƒ}¸'?ïŸÂÓyº+?xã‰QuÝ?QH£!­?B°—¯VÐ?…æ6ÁG‰?w³ÔóRê?ïRHððÕ?•ƒÕÂQº+?aïʐ¢ô
?nÍ.*
™¥?"ˆîNó?" ®•ô?î¶c•ëS?'ŒÂÜI@?j{×D%›?dG%îNG?¢ò	0üb?ØLefê£?ìÅ<j¸?˜©©ý¬ù?v†ËGÃ	?fy¯C0ô?¸m¿™>S?˜tiP©û6AGN4FGL J0039.1+4330?×*²zTô"À3M½ÙßÛÀ:¾ü‡7À<žÿ%­B@yl®)@
  ôØ?Äa1s?'½?Ú6bÂö?ýàõþõ>@	·"W`9&¿ì²ÊÃQ-?ïùZ"¡U¿á­,ˆõ¨¿Ýe¿cØ¿à/³KòG¿ïÿ8"†ZAGNbcu3FGL J0039.1+4330NVSS J003907+433015?ïôŠ²\D`?Rù;°Ò:¶?>!»ÑyÈ*?E"f{/ÿ?NÄX¯Š&†?HS¼¤Y/?ïçÚûlP?móF¢vp?4ö§"Ë<¦?B½Ê•Ç4È?e†/n|ô?jÄhù¶^O?ï¾¼8ù5?ovvãŽë£?Y¹™£Y}Ì?h0ÈÀ
Ï´?z3}MŽU?d7Cè%Š?﻾çÎ?ZØ{"kA:?]8‰ÒG?>ÄÀ°{?zÜ>I±¸Á?Y–q½MÑ?ïî.Å¡p?S–N,Q h?Jg"Ä™?@TcY-¥?VnòùʘR?M¥ú[?ï²µÃWs?"'ë!ŸÙ?N‡¯6ªH›?_âä5Ô:?j-wõ?'é	ú@ט?ï—9´ùé³?wîˆê5ò?_íw8"ú{?eH$eFÍ
?†3ãÝ4£÷?u'|wpû?ïSýÜËXÀ?u¥Â$-Øë?på~ãÍ|Æ?\ݺ°À|²?'F䪉âà?t¨•E,AGN4FGL J0040.3+4050?Ñ*e'潩À5ü¼ßï¿@À:¸Ø£š¤À<zøØÄQÔ@!A߇O?ÿ¿ "_õ?·[±×~·¿³0M¿jRs?û-
ê¤N)@b14?èöIØÃ{¿â6M™æÆs¿èê"‡¿R¿Ö^¿à12I(h¿Å"§ŸÁ¦ÔAGNbll3FGL J0040.3+4049B3 0037+405?ïÐD¦x$T?j/H‹í±	?@AgÚJ(+?/ɗD5m?uÕª®_'?i%ҋÌQ%?ﻶiÞëÞ?|;êá8«I?Qnü>TÑu?^1 ?*Ú??}ÉõF0˜?y/ì1
ß?ïi[sn6¿?…•Ôbú=w?Uð§>ë?TAChߐ?'"2Ž¤qZ?…tMH¡ô ?ïBÄA>–?zî{>«ß‡?bv{ÉXZÖ?F»ý»ø?•X¨[Õóû?z׎‰}'1?ï§h–¹·¿?y/¾`Ñ?PÓjÉWŽ?C¥£/܁|?"z1Ÿ_V?w¿à»L2è?ïO[óÏM¹?"•u‡;$?`Æ?'¥Ä?m…"î­ôÐ?"û¹©—Y?'…"ù†?ï­¢B¾?dThb?]áÒô¨5?Vbù §?¬9¶-n»?#
øÕ´ë?í0ž±V?œ0DïéÊ? ‰ÉÖû?p‹'QJB=?´Vù9{òv?œ¾Gº.ªAGN4FGL J0040.4-2340?ĄMóäúÒÀUo@öjUÀ:˝_÷·À<š/²u2²@ÍÛLlj6@v¿yýòà?Ædô5òUH?ª"Ù…xO?ãl Åre@3¶-y
¿ºÔ뿬'ç¿èk"\Ì4¿ã³A
ŒK¿é}ÉÄڐ¿ÉÕdK3'¿ïÿס<%JAGNbll3FGL J0040.5-2339PMN J0040-2340?ïÒ`"æ›?k[¿
mÊd?>Îy…éÊw?4='IÌ%?tãáú¾?j(ýSk ?ïԜ÷"n?{'Ú_;â ?@YCËí"?Ib™_Héƒ?s¦[ê!Ÿu?yɲ'dMQ?ïXí—r¢à?‡"
uP½?a9HsPÍ?m:ù­­Ü?'»#ýÂ*`?†6;ÒT.?ïÞ)é³bn?P˜‡ ÷A?&ÆÁŽæš?ö«|P?p4Ú–&6?OËɑë—s?ïkŒqq?‹n{öªó‡?Uý'/‡>?OQöK®'?'N!~9s?Šiy¦QÇ?ïŒlÊP4?"…¡€rõú?P¶UÚڃþ?^fËÞ\¹Œ?ŠÎ¤AŠ±?'Ù{I
.?´'?"ã½[?g걯Òûl?lsV'y\¯?¢à+øw¶?"¿Ð•"IS?ï•Bˆví®?rkÞe?=cþwH?58ôêdR?‰ÄDïÇnV?r6äùAAGN4FGL J0040.9+3203?â+©·§>À>Ä(äû—»À;ðR
À<]J]ò$@Qmª'†W?ÿ–»cýM?ئËEäß?àEÜMsPZ@ÙÂbæ@€ðâUË?ïøIóiȿքÖ~|\È¿á¬btx¿äÏìÂ5š¿ïØl:¿å5{!ŽAGNbcuTXS 0038+319?ïe³p
?…Óm'äûk?m*³FŽ»·?cnÜ]Â?rfTÜ?ƒA8xÒ,¾?ïA)RV0†?ñÖK'n?tÝì=-?vÙê,Z,A?'©î;âx=?†¹+uÈ°¾?îÞÛê:à•?Hòxˆú?ˆì^ÄÞ ?"½¹<)Úx?—®v
ùL??‡ãc7ì?î»"wNt?x×Ö^"¢{?TW!ÒF?d-̔ݹ?ŸÐƒM˜][?u~øîYZ?î›GLMi?œ*˜³TP›?€¾«xžŠ5?xÁôfÏ®Þ?¢à]ݲ¡?™î'ðÑ2?íú|,æ?¨¶¶/uF?‰žæ]ã"3?– B'7)×?©öî¤Üðf?¢Y×"?îvB㐚?œŽËÛXà?'ÕG·Òÿ?‹M,DÝG?¦Ô1,3>æ?—Rð2š–?ìÿHé›(?"O˜ý9Ÿ?‹
j[Dr–?N:;ãJ†?´¤jDÖï?'쌼®ŸûAGN4FGL J0041.3+6052¿åðÓÈrí¿ÿƒòÖKÒÀ9šN³Â9ÌÀ;Jˆ0»‰®@5T#sø@ä¬å¦¸f?ŲºÒÏEM?áúˆÇº>U@‡žYòº?öY0³Q%·¿Þ–ý]
w7¿Ë$úì.'¿èÕÃ"æ¿îÎR]ðÌ¿ämÊ=¦S¼¿ïè/>\;AGNbcuNVSS J004058+605407?ÞÙ¡t·ër?Ǘ@ï'ü?Én—üû, ?†»•p¦?ÔoÝ^ü?Å!ø"7Q?ÂLm¹8gÈ?À- úT"?ÉrT6Ê'½?Â67,?åOƒÿ\?Á•H"±³Ÿ?ÞvݕO•?´õ¿´É;l?Áöï,•©?©ï:'TP?؍ªÓRÍØ?³0͂Q™?µ•Ú&º?'ÌՋVB©?Ý|­A¹€6?²Të[™ˆò?ÝC=é›?°kúXƒ÷1?Ô%Á5ŒK?Ä£ˆ¨'?Э¸|€%¢?Ä2ÜtT?Û-7ÂJN?Ç.ÇY¬á?©Ö!<@I?²&¯½k‡˜?Ì)EÊ@?Æ7/}WTâ?çXZíZü?Æ)륙ÆÕ?ÓòC&ÎÔm?³áÔ s?ÄídX*u?¬<™õŒu?áã'‹-?¶"â§J?ÈXpoÙÌ?t¶Š9p?â$e¼M?½¨»ØU8Ž?ÚɎpèí·?½
Y¾?ôÀMIXED4FGL J0041.4+3800?Æý±Ï3ÉÀ8ÑüÁr&À;ŽK^À<©G_ɔ@ ÉfI
5
?ÿÉT!ÀD(?ÀU€ÙÚ&¿­§¤|ÕX?ï0\S½í6@½ý|(?쀏qøjà¿äŠ:N¿â֘B"пä÷bØ<l˜¿ÕœøÞbK¿Ä1ƒìÅLAGNfsrqB3 0038+377?ïÕÆ÷€Ä?ƒ«S€Ø6?BQóà¡×?FÈ!'ø?)?rÒ±ø'õ×?'VÎ1š2?ï°X×vbÍ?'§ð÷Zß/?U…¨EPî?\¿¿•yë?9,-v®?€›Ìt™LE?ïd^îð/ ?€Ô]·®"?[Ð;?Pr|©Þ³?'· ÛEJ2?€}w'"g²?ïu'E­øæ?sŠ¡ó"?Qßg‡Þd?:ávƒ' E?='e<e?sŸ–ío•?ï©ÐóÅVƒ?w873y#?Wà™|K&°?KQÌjð?'¯ÑbŠn?uvÿÒñŽ?ï%énC) ?–BÇæ}?e­PÆüX?w:ÌáÅÚL?˜(/¯r?"t¥2/?îäŠhE±?‰Äß·`)?g2A]ki?fo×肊‡? D5h[wå?ˆhU;â'?íí_ï|á?•õ_©c?m"Àð´?`\Ù sì?¯PÝ#mS§?•öOwîk\AGN4FGL J0041.7-1607¿âÃÃÓmÀÀS±úëÄ	À;±¨´¿ÍÀ<ÜøÆOÛ
@!ËXàÁÌ>?ú;´4çh?ÕغEºÊ?ÇÉFZ'W‰?öIŒ\`S@DÃàj
?Ûö'¡þm?ïúeµ²¿äå\{+‰¿Çܺ–}5¿Ë­šW"¡:¿ÖÖò FAGNbcuGALEXASC J004141.24-160746.6?ïʒEšòh?o‰±8Ùz¯?B›ÇG?5u]¥é?xsI™Á"›?nLÜðcf?ïÏRÅc¸?yÞ38Óç?I•Ô‰¼;§?VœÜVÜ?u#⧏Y"?tɋ]ñi¼?ï3†(?‡BfmL}•?[7¤Ÿx^?TßéPµ&?—Ô4öø£?‡Ü;½‹à?ï'M™!5?t𰇔ÚÓ?BÊf!m?2Éå¿`æ¬?ŽS<yÞ?tŸkˆ–¿X?ïQ·á5î?@BÛßɱ?R•Kƒòuv?FJìŸLö?‰Øè¥J›½?}ú!uMŠ?ï‹z‹G­z?¨$¦òUo?YZíI_"?va¡L?Åz?Š'¿=i®?‹ƒzØÀ^?îüS3iö?'¢£Ì!?cSæhs–¯?f2QRÚJÀ?¤êüf,)¶?'š@ýY=?ît.Žïا?"~=mÒ?TmˆÃ*[!?N`)™'¨š?¨ªÎ"¹·?"'Î]îAGN4FGL J0041.9-4702?ïNÑ«–îÀQ­À˜$À;ã‰>ÃÀ="ÏÝù@ Ÿ³-¿Uì?úõp	}WD?Öí!zN%?ËD&J—}á?òò<ÈÞ*Ã@hÍ¿ïÿü¥¬¨¿ä¥AØèd?ïÿê›ê¬²¿Ýó"Çz¿áY®Çÿ¿Þž¼n/ÞAGNbcuRBS 0097?ï³[¯~2`?ŒãŠ6K×Ê?:?:b•?5JK9êîÍ?'Y36½D?Œ¼¥:Ì)›?ïԛjÕ
?vÎ穦é?D]‡#Y#B?LbI"[±?s&™Ìä,Œ?szÆÛG?)?îH	µ>?+]j®
‰?{Ó3|¢?"¯ƒä?¨94kb?›Ñdž²yI?ï§äsî m?fr<×?7_®Ä'5?- Ýçd¾j?…K冭Ø?e°Nªg?ï®01œv?ˆæïPâ?D¶Àߨá	?<5CÉ­4=?ƒ(‡·°ë?ˆ°ùy×q?'ŠÐ?ŠÌÓòNõ?T'4Ï+S?cØä£OE?ˆ‡¯§Ç˜?ˆ?y"Jã?î	÷—á? &—=?}ÌõӊÙ?"Y	@Ñmz?«¦çր8?žPÚ:(?ï3¬áŸî?ƒ®Ñ¯±	?<P9'–šµ??†Bë«?™-)yŽç?ƒ{Í8R
öAGN4FGL J0042.0+3640?¿gÈf5¾ÿÀ:)/ ×{|À;ò×ùP¹À<Fyaî@È)NWüÁ@ç';®+ø?ÃD&àêf¿ªñ/؊Æ?ËA˜¦ªy;?ÿ¡W¾'Ý?écànë?î¨ü
,8m¿ëŸ|!Ž›¿ÑÎû%OÅ»¿ßÍã£(
»¿á¶Í§%sAGNbll3FGL J0041.9+3639RX J0042.0+3641?│
È?pŠªpZö¼?IhЋ4²R?@ÍÉtå?|þÞúÅ+4?o1Hµ™?ïȗ#{7â?s"ómî?IÈÌ°~?NJNC4&0?x"5 Z'é?pé¥s‹Æ?ïETh7 þ?‡D¬Ž[%?`€Ý†"}?OûÂìF•?•EWKa|?‡Š}u`O?ïqLpÆç†?n¤SM,H%?nõ1G±&¡?T£*6ìC?‹ï—q?kçoç¡À×?ï"EÑè·Ü?{pÀǯÑD?\µ^
h3ÿ?Soź{½Ä?‡WßÒó^Z?y( J|?ïcvYÎ}|?Ž(Ž[ÑK²?W¹Ÿ†^! ?a‡q"?ÕÚ?'šÑ:
a?Œ-Pp/èÑ?îÖ?1™*?";ÉJZmê?gÔl"kø?eÛ
4â'?¡!ZøÜæ™?'«a9£1??îyIZÅ{þ?‰ØJ¶/òú?…ûÃFÈ.?s´Fçm©{?¢ì¥àBÙ?‡ILÂSá¤AGN4FGL J0042.2+2319?æI…ýQòÀC¿rÅz%À:#ŒÍ}À<b Õb"@\*2	h@Ö×¥mã2?¾‰_d¿rF?¾Òo_DšJ?ýzŽ ¿"(@ø­ˆÛ0¿Ÿ»Þ#G"ú¿æ²g'Ñ`¿ã$e¥vF®¿äšŽ:!¿è@*'_–>¿ïߏ@zAGNfsrq3FGL J0042.0+2318PKS 0039+230?ï±¼";t±?r}ÜngQ?V9WÍã$?N
/	ô?€É´o¹1?p¦UòË?ï¡ÕÔø?€Ø`ø'?Zîµ@óG?_rQhÁÍ"?"]óíúL=?}&«Äù›?ïoß«§'?{ÏÎþK?hM	©½P?hX³ÛH?ôÒÞo±?wƖm»R{?ïfÆf½_ƒ?i"†^"»?u¹Þî?QÎéöëç•?‹ËÞ[½Ì?f(‡n*ùP?ï¶×~<Ø?'õ1Ӊ?ß?{àb¤•?|Ú%¦†Õ°?˜¦ìõS'?Ž6Ï\å'R?îä	"/œr?—ŸÚøÊܧ?lhë¤êµ?r@20
Õ?Ÿñ²4Ï[?•Ð»©?Ó?î˜`hv?•Šö;ü"?''–?–r?6mÕdƒµ?¡÷IO¹­Š?'oWÇTL?îØ^6¨D?…€ǿ‰ ?‰y¼$Kg?p)6³Kî?¡¤id?'=!›{AGN4FGL J0043.5-0442¿§´]ŠÅÀPߊ\å´$À:æ~Ä+=›À<†,:ñn@ š:ë
š?þ Aׁ\?ÆÐ\cÙ`?¤âcâÓt\?á­»úíqˆ@""xB[ð¿ê?.8¿âÑBþ,kC¿ã'·iŽ9¿Ö
×YÉ¿àý­_Ÿ!ï¿ÍïªGfÆÞAGNbll3FGL J0043.5-04441RXS J004333.7-044257?ïã_<Û?Vpnˆaùp?-Ô££ïùÌ?'©IVé?k VXǂc?U¸"_]µ?ïÒכæX˜?t¦[éq³?DŠý`ã?NP˜Í_WP?tÒtÙÕ?qwWiç+ö?0Fø@?o˜ƒú_?Yøhь?RÈË]؝?‰qä?d'?mžW˜$d?ïT¨C*¢?q~zًß3?LØcѤ?5yÛnÉÄ?""4yü'°?q`ò½Ë?ïÍ¢_»ÒT?fu9žúZ
?;+)¬Ù?*qKè_"?w|¡9ó?e­¶–Þ^?ïx•"¿ ?Žlá{"ç?X?r‹×œÜ?du"õ£?Ž÷ìCPV?‹èŽ§×›?ïB¿–ó?€cÒ¢äû?_ž(é2?M]«'ã	?•Å¥wYŽù?qíf ÷ö?îOʇg?kú3"*e?b´(ÒaU=?VPËÞ ?®¯ÀÎA
?~æ'.ÁAGN4FGL J0043.6+2223?ØEFÌÿ2âÀD9‡çÀnÀ;¡"úÖËÀ<'g†!Ñ@†Ã>@=–é»ðÜ?Ò£9UŒ$?·iþ Õ®?é=[?Á¶ï@¾†ù¿ïØ ó•Žr?ïџD~_¿à¢wžÈ·¿ß.8øo¿áéBžá7¿ïþΈ°=AGNbcuTXS 0040+221?ïé0!Ó0á?RótUa6?0X‹à¯? ž%K2‹j?dÄÌôH†?Q>Õ§¶™?ïÚü]çša?oýñáòâU?9é€[É7?E=Ñ»¾S?pã9&ð{?l}_>cnä?ïûRÇ">?p¾ß ¦Ü?Z—.{¯¡?Tœ'£;?ˆ¿8X™Æ¦?mÛ…¿x?欄7wªJ?a‹a´Ü.T?R¡?ܶ
;?6 s¬Ð­?""Š ³Û?aKÕê?ïÐ~ŒfÄõ?g5'…6N[??´¦Ð|/?0àƒRë?uÏ>žûž?f[Âr"«ª?ïŒï£L±ñ?†óà̃ݸ?JIUam1?\ñÓR'*?‹†ÓÐ>u?…l2~
"A?ïFŒà¤?Ø««I:?aÑÂuõìQ?RàTHÁŒÀ?•á1?~—Þ0+?ï0—/˜?{
"$µ?]M8½U?M÷ì?˜)ŽC'²?zŽõ€E¾AGN4FGL J0043.7-1116¿ïD"†YmQÀRƒ7u¸À:șI—#À<ˆÊ½ÿ@ )Ð3Á?ùz@Ù#¯?Óì'?
?Ñ"‰âíJœ@¢Pr[@}¢×/ý?ïÿŸ¸fä¿ëa¯ÐâÜ¿Ù5 uÖÇ¿Êò*Z~&¿æØåÿùŸê¿ã‰!Q^lAGNbll3FGL J0043.7-11171RXS J004349.3-111612?ï¿ú]öø'?†ð®-™N?8b´…'œ?0¹b"mõ¥?~yúñ9?†ÔDX§¤?ïÃÍ»ìð?}žÊ?PO4¯:vu?W—Á¼q4Ÿ?zU<cØ?xې¿íI§?îßg°#¯ï?'°Š‰[?hõD/á?qT0Pü,? z0³&2š?')¢n]w?îç>
_l«?y'süð4À?YMùß´ÃÝ?C¦z`±C'? Á¯Xå͹?yAq"H?ïvàéS/?ˆå£Ç띐?I̦æ]¥?C'
ÿ€J)?U}Ö
j?ˆ]:]žK?ïu0Õϙ ?š,*o.%?]?ÛL–Ur?iGW†'in?Ï#æ¥k?úÈì?K?î1Öג£†?š€…¶Åc?k¿ƒ	s"ø?r U_«Õ½?«&šXYË?š8²6(?íBO­BŠ?"´S#D?d…¬š ³?Z·Ÿ…î]?µIU5³ãi?"°NÝ¡AGN4FGL J0043.8+3425¿Ê¹IÂì¤.À<j|¦CÌÀ8b–›¸XÀ;'U¤wC-@^[/¦Œ?ýÓèPïÝ?¡kÉýQ?ªs‹_fN@
¾•ßе@ýýÃå~?ïÿG©ýd¿Ø\4ß/ÐÓ¿àíØJ¯P»¿Ù·ã܈׀¿âÝÞQ"'¿à°éAw™•AGNfsrq3FGL J0043.8+3425GB6 J0043+3426?ïíÀJ»îŒ?QÈ{dfeF?VŠO Žm?ë£Ùä´?a}Í("ý?Qi™4c›Æ?ïé/
ߑ ?h	õ<!­F?29™R€HÖ?@ûWE´6}?d‰¾àóñº?eZ«óetB?ïv×Áâ&ë?‡áPüí‡ö?aGº>ØÀd?j³™ú,Î?ø ý?u%?†Ê
†¤•
?ïД6G(¢?Wö"SÌÝ?8™Dæ3--?!W>6ü@?v,Pªå3Ý?WHäÜÞG?ïÚJ‹‹Ü9?eY
ՓgH?%)ì¯d1?†$3öY?r1jΆ¿?e
)šõ6"?ﳪ2TLD?"dó´Ê¥?P;žs?l3øPôc?
ÿ™"j?'–Ӎ§?ïk4骣?‹^'¢•?`ùöù¶'»?l~–´9‰?z#ÿÛå;?‹ñJ€c?ï¡&#çL?qÔä0\7e?G)½z1¼ì?7C¥#…m?†CÛ2Qr?q~HÈ­@³AGN4FGL J0044.2-8424?™q=—ÖšÀ@\¤~Ïé¸À:P"Þ™À<:Dfa]é@Ä9Ö:Š@JCþ\'Ñ?À4	òÈ	?1SW''»?ÐU@0ÞP^¿ßB™¢ÓÔÿ¿á€Ì¥Wh¿èˆ^Þ²¨¿ëÙY_ç¿ÇbT]û2ç¿ïÿ`}™2ìAGNfsrq3FGL J0046.7-8419PKS 0044-84?ïõO[÷'`?Nî̬Oôä?,Ԉöð|Ô?+h¼Àé?QƶqçZ	?Lˏ|TÈ{?ïæA·ýª2?pvI}`u?0pø ¿á£?@¨EgEÅ?g°(øTä?nüÕA?ïkrßñl¿?"xXG:	e?WØa=Ð ?Y£Ø4#'?'¦|òh?"_Îœÿ?ïô%K"ý#?8jv\'³"?êæ|‰>ÿg0³kj?V¬i©á–+?7¶‡'í
?ïæ°5'^?gÙ¢£¶?AQÿ9•_?Dµäqùc?dûJ°õ£'?d¸I˜‡nF?ïªÀ59Ȥ?…i07ƒ¹ƒ?<-)‰¢­7?M›k%ÉÛY?"n‰pb°Ó?"ÐS@Ï?î͜§&[E?"D'lˆñ?f•™óÇ8"?lì²tÌ¥Ÿ?¡¼Ûí?ø­?"–Igƒñ?ïܯŠ`…k?Y1•RU?*G•ñ? ÊÏ5«dý?pÕü©Ø?YXh^{AGN4FGL J0044.8+6802¿ïR{Lý^»@²{²þÅmÀ9ÈÇÜ$YÀ;¡óÒvZ@ו#SÀ@N
Ää ÿ?¿TWñ?³S¡èÅ?õÙ	†'@éšòŠ «¿ÕßGŽ4
Ê¿ŽXkã=í¿éùù î?¿áx7Ÿ(¤º¿æPqgKh´¿èë»MlšAGNbcuLQAC 011+068?î~ƒä¯E? ¤¦	‹çL?h§3Áf¨?]ñ.Ø.£?¦–§Dÿ˜º? B"r´}?ëV?XÊ5]?´"7/"6?wÒkìù?{QQ¢¦/ï?Áèo=ƒ å?³ÐÌvùÊ?í'´cc@†?¡â­	Ê?‹A.0#?ƒÄ©ø¥+?³Z7#żi?Ÿ$Eu#?íDÞÔÃv?…¾Šà[Yt?…*hÏÆS?akEæĐ­?³3¼F_
k?"m&ç"ù?í‰òñ?²Éübç?yòH:aá?vNdڞ€?µì‹ë"h?±ÉI"$"?å¾s3‡?ěd'¥i?û'E?"4§ÍE	ù?ÔÎl
Pw"?ÃÑqĊÖU?èþÕ;Â_?²doß>œü? ¹Žœ.'?–!Þö:Ç?ÇÖGj!ÜÊ?°¦%V"N·?è"HÄ¿ã?ž·K`o,?ŸÝð3úÆj?¸'g?ɳæJ!a?œUû
`ƒAGN4FGL J0045.1-3706¿ãQ>܉®?ÀSûί%À9µ@+i:VÀ<†ãlK'µ@çoÚX|@¡–EQBé?®©é…Y?™€öà^?çœAƆ@†¥ªõ·¿ÏȆŽàÙ¿æ4B'KÇ¿çÖø4Y£à¿èå—ží–¿ì '¢ s¿£.üÓТAGNfsrq3FGL J0045.2-3704PKS 0042-373?ïù¬«çq`?<ñl0m?#·ÙCø{?¦°	&ÿ?Dia'7?9
ŸÜ´r?ïí"?H¦s?g¸¡hcJa?/Ué,ĵµ??ÌÿíŽ?`wb@s®ë?dýØH"Þ?ï¿(v­Ó?q™WݓÙ?Y=)ê|?ePoèpñH?zƒW«f?kýG]öw?ïül$ôߙ?#|dĖ˜–?Ìôjµ?ƒ¦ùï?7zæà#2¶?!‹–Më§?ïô¤Þ'h?OËËnw?,Œ®¨¸.$?"֙W¾þ?S$¬¿œü?L@ºžÜФ?s%^?ƒ~*4'k&?CÉݖ<Úf?WÔïêç?|9æú¢'p?ÖÎP?ï‹GD?ӈ?€LRÜvY?`r"›¥±Ú?iÁ¹=aÖþ?‰‰Ã¢Q…?zùáMýTÐ?ïö©žZ°?CÅÀº´¿í?0†€^Ý3?#ÿ~aO"?O¦VUé?A1øŸAí{AGN4FGL J0045.3+2128¿¸^FàÙKÀD°üó0À8Ýi¸*~YÀ;œñ-Õ%a@¤zŽ¤h?ú´‡Ç	>m?¬º¢}ÃÐ$?³ˆ¹ø^Ëè@ZÂß
A1@žA|Í,?¹Jˆ ‰3+¿Ø/õ;*ùS¿Ùåpݍº=¿Ño¤}£Cç¿â9ʑ‰)à¿ÕT•cT
HAGNbll3FGL J0045.3+2126GB6 J0045+2127?ïïbaQ²-?‡Á—4p'=?nÁ£³‰œ?@.l"?_TQ™ƒQâ?†É€ü"$?ïëcd9¡ž?dÎ
 à*?1*³`ò!ù?@¸<k:3Ä?bwE4Q;=?bMR§@mþ?ïƒäH
þ?†è9øÂ?_
?\?oDCÓsÂá?‹%M±'™'?ƒÇËöØøÌ?ïÚË>Æþñ?Tú1Hõ)Ê?筊a/?Dw

æè?r%üóÁèG?T¬éì¼?ïðÔ,×=X?S3_}éå·?ž	/Q?~˜ŒU?\}ÆOë/Ð?Rt(JÕ{?ïÀÊêÒ3?€>m2G§?G•'—<7É?byíª±z§?|§Ø·<ÈØ?}â4ìŒ?ï_§õŸKW?Uwfúò
?`Øðù"d?ošÞeC9?'ïãNÚ³´?ŒO'r4¤?ïµÈ (?l2õ6'£@?*Ç2Í<6?µjÕj?'O±ƒ'+?kðxÉ£v4AGN4FGL J0045.7+1217?˅îC6'ëÀIGD#‰À9QË(‡Þ†À<IbI¡4@¼ÇÞ{uí?ÿPUhaQ?¯<òN¼{œ?•(%Ž.?çs÷+E(@ÿz'î.Ç¿ØPQÜÁŒ}¿âI¾ó(¿Þ¯îºÞ7Ù¿à')ÜÓ¿×âš~ñ͍¿ä[³"ý*cAGNbll3FGL J0045.7+1217GB6 J0045+1217?ïó2H–`™?FçÂCd"?%âà•m™B?V‹öþ?VßþjÀ?EAeLÖ®?ïëªqòÐ[?fõ¥q[½a?.ò³&?<ñ²ªmç±?bfeµ]?d€óéÇÞi?﫟ɝ?ys-JA;ç?QÓÖ¸PAv?<ß4˜àê?'Ý'ånÝð?y'
6·8?ïÐt3¥ì?U&L:V@;?5®œ;H
£?vQÝo?v\5LËZ?TOkýYQ?ïãñ×$®?ad'1-TŽ?9×ÝÛþp?/'òQœ¾J?hÓäFýœ¤?_â׫A¢?ïÄM‹W?'_÷ÖøŠ?<ÆÉz»¬?N}Àz??|1@u I?}²¬©ƒ~ö?ï|½õ]S‡?'h3b«?WáŸð³J?W?n!0þ?Þ†zÜSÎ?'åÑVM'?ï'ñÑ,ò–?q
ÂtƒÞe?GêóJ–áô?5¶;u9š?‰Ä܏ù·Û?pÓÐ;cAGN4FGL J0047.0+5657¿ïb…ÔêžÀ 2@Äì.À9'RYi'âÀ;áJóCY@Äé÷U @"úC'œý?³õõ d4Ä?½ü`‰ê
@	,žÄ{Å@ý¢Žø×?Ôy™ž÷ýR¿ÔúŒ"¸'¿á»´v"±Ó¿Þ­' ­ßø¿å`s^™¿è fèlAGNbll3FGL J0047.0+5658GB6 J0047+5657?ïßüÏQ•?YÐ?Í??@½Y 5Ãý?2Þ?…Ô=?l¹¬ç¹?WâUóA´?î¶
OLˆ?¦¾þg€k?E'i¯—.?U+MLk=é?¤JòM­
y?¦]ÖÜÜi—?ïZ"ÞÏ?Jtž‡œñ?fôO©0œ?au½Å뀛?'ÞQÄÊû?HlKÉÕ;?ïŒé*ý?dÅ}Új©ö?SæqŒß?4W{"c?Šc{´Þí?cžÌª¯=à?ïÍâÌY¤?eVמ~-?Phߊ8+?HìC{ä'D?tô½¤S(?bÉtòÃÉ?ì:–I-•?½
q!o*I?UiÒ$?hl
T/a×?½Õ©¦hEJ?¼×ã@׋˜?îð‹V=ô?Œ
	Õv&"?rb1¸³´ÿ?pd¡~6/?VÐR 0?‰Ìñ€xoÚ?îÒb{[?D¾'E?hôc©B?R2Åöâ?¡J'Š?€|É?]AGN4FGL J0047.1-6203¿ãyIbÓ"ÀKˆÎp:ûÀ;3&yÀ<‰ÿæՌ@S1j0Jv@	]"à¤ñ?هö#]RA?äiTpš?ú¡#K^£$@k%mL߂?嗀Œî;¿êŒºùe²¿ïü£õ=._?íSÀì÷¿ïZ¿Ï
o¿íã°> ÍAGNbcuPKS 0045-623?ïá$ÙºW?²ïQ¨d?˜¥†?}L?±"˜\eƒ(?tùT†¿H<?†<÷U'+?î³wUì?¾OèÈxL? E"»Ka?·(šç˜H?œŸYæÀÒ?©'•.Éï?ìNˆÏs?¥	¿Ô8Hh?£±˜[.?—¥n[t½9?³ýà¸Ìk§?¡!Õ_9ï?ï%(@ïg	?"R¿v•6?uŒÁf^¦?G.C³~µ?…ÊÖ:zHr?2Ì9`À?îGL–ö?ý?»S~"jÑ?©4ãtt•?»U—e{ž¡?tX
X¾=)?w'K	|J:?ë»Ôˆi+Ï?ÉédvæÕü?³ØÐçs?ƒÊt¥:Ú?¬'«×ž\Ù?°ÚÓ(d*Õ?됲)ÞJÏ?§"	©:æ?¤ôÔËñF?™ÉƋ~ɖ?¹K'ú
?£Í'q¦8ù?ê&õåÊʔ?ŘÿöoÞ_?ÂwvÀ6øv?ÆÅï|‰?£²ÆŸã¿ë?¤õ†@«©­AGN4FGL J0047.9+3947¿îL~Lƒ‰À7¶o"5ÒÀ9uÓú¾wŸÀ<*¯ZËþq@¬Ë"œ?ÿ1è_ÐJ0?­óÆB"?œi³Å6Læ?ðw_²íþ@»4‰tˆh¿Ñ	£¢†þ¿áHÅ †l¿ß®¬:Ûô¿ßj
 AÿT¿Ûä:|¨¿áª	µólAGNbll3FGL J0048.0+3950B3 0045+395?ïò;Ëvû#?p'=K'Œ?,¤
×Ñk?FÓ4ìâÇ?WóçÂJ?k«QÉ<œ®?ïíkñÉ9"?f"†×z?+ڎÞû$Ô?:&ƒrjÇ?`Öe7bë?cÿe=ØæÔ?ィóåђ?m#~F™LÜ?QU
Õ«ð–?;þòëßì?|ÖB¨*Zä?l[»-æ1Á?ïÛÕ`;¡c?O³F½«-à?4ï1¢2R?eJ°³Ûê?pÆ\àž˜^?N‡³Ù–…_?ïå5¦woð?s3'÷<£§??
å¸*>?Jv7i½?fèü߶GÉ?pë;ˆþR?ïÌ?ç ¶?'»…k~!?8ŒïÌ0¸?I¼•tñ?xW=gã=Ð?'Èí×Jà?0´T?|xÖàå¨?\EõŸ(J´?Y.·;«¨Á?‰NµH5s¶?zƒiX•Œ©?ï§
»šËH?l§zaÖÃË?HãýÃ%0?5¥¬a:'S?"¯7ü>×?k)!ª©EAGN4FGL J0047.9+5448¿ïزކ€À "q›MÏÀ;MHœQÿÀ<¥;Ϲç@#—/£†­Y?ùJ?Ú
¢ñ?Å …œº¿tˆÏ-5~?º´÷ Þ@íšü?ç–º$Sœ?ïþ¡ÆŽÅ*¿êZ^gŠS?âúÎÓ7J¿Ý=–ä]$¿ÆÑ>¶ôô3AGNbcu3FGL J0047.9+54471RXS J004754.5+544758?îH·3³`À?§¥FÐ7Õ?Wù(8ðï¼?Tƒ(§0¶w?ª´Ã‡!ô|?§O]Ÿ
9?ê·p†È(?Äçòw\®?ZüÆ<~M?n\J§Å¶–?ÄìE°Zț?Ä´ú¸îI?ëäj¯Ï?¦pTÊ?qÆj;ãÕ?qj×ãvõd?¿ÀCßJJH?¦gW§+´?ïµÇˆÑ\?ˆj¹
P–3?h¨ÅVða?\õŒ§[Ë?™´.dO1'?‡v7'R'‰?ì~ËûŸ%Ó?µfݪßu?q>(×}Š?nØZ\0oA?ºõ½˜·Û?µXíG¸?å;^TÁoÄ?͚|@uïy?_.'%Î|?qõo­0Ö?Õjә+?Íxƹßú?éžÌ8EÓ?ªðjé[bw?|
¦PË[?y9ÇháB?Ȥ`X@š
?ª×M%W?í
7"Ž?¥O›*µ­™?‹Olh¢Å?Šó÷RFt?´,UÒÓµ?££ö7É(AGN4FGL J0047.9+2233¿éËÅXHÀD&™Øƒº4À9àGÐy)¸À;é•é
ðõ@H	 <Ëã@åäËÇ?··Rèa?Žá‡Ÿ¤©?ØÇW­eÿ8@UC#Á%O?ç(å!,u¿å˜|··ð¿è¯;Œž"¿â13~²†¿äñˆ£¨U¿ïþÛÝáÈAGNfsrq3FGL J0048.0+2236GB6 J0048+2234?ïùÓòõš:?8ŠÙ[±ú?!µ¯u2?4LÒP›w?Dia`ÀÊ?5ɽÌU?ïëesøa?gM>T×ü3?%ìAn?5"4C²â*?c;ÇÐ
q÷?eÀT­Mõ?ïš>ë"?|2¾/Yk£?^Àq+æ?c(Šä¦?…˜}€Wù?y]hDŽÛg?ïçÿíÅ?GÚj8µ?"žfAOn?
´'ðÖ°T?fÖ\Ðàâ"?GcàÃH?ïöH"Glj?DC:§š³?+ÑÖwŸŒ‹?ԆSú	J?Oë·ÙTS?Bi*݅ç?ï°µ¼²DÙ?ˆ¿ôˆcÍk?;Òé½òx?Sz·ò™;Û?'ô¥¼Ç'?ˆŠIå?ï<Í$ØÉÓ?Šeü˜žEF?mw/j?qa¬¹K+ž?"ÄŒy…?ˆ–íVõv?ï·­¸›¤?kLZ?Øv?@ugË<M?/ô5 «…?4D`C?ý?jw:Œ'rAGN4FGL J0048.6-2427¿ï+҄zV;ÀUÐQ£"îÀ:×{‰äðÀ<¦WF7ò¶@Dú¦#ë˜?ÿ¡¸·lx?Ä~´%Œª?º5‡Ì<¯?õ®žä\6@VÇâØ'?ë1` (Õ¿ß[dc¿àgN"¢Â7¿á÷7…¨K¿á¥ø¸
"'¿à_`îWaAGNbcu1RXS J004836.9-242631?ëëßë@?Ñ(¶¿Á??;"´iõ¶?0ÕÂÖCO?Ãвµtk?Ñ(=çO"?ïH0|°¼?¦3ø^?aö
+3‡?sRßë?"À˜J´æ?¤"8å,r­?ìÀëm ë?·¸*+Dç?XlÒYˆ@Y?J>¹¾ÒV?¾¸EZ–é*?·Æ;ÃÐyÖ?ïMç(ž?r[YË)ð?ZĶ	³#V?AÜOŠù?"–Ï¢°'±?r²#XŠ?íߚYÝí?Æ] Y§;C?bÕÃ'çã?k@gB<7?¶šUÜ
W?Æ÷À&²X?î´;9r¬?±âœåûÞ7?kRÚKp*Ý?|;ã)1?£!hw¼?±)\鼦ø?ì7±8,þL?´ðì¹<§D?d2Ct
?UÎ;Ó«?½ ä&/¿‹?´ô¥,?'?í夠™ú#?ô)'ã?pZ¿"³Î?^{Ö¹UcÄ?¯š^^Ý?ÀnÃÍ·¾AGN4FGL J0049.0+2252¿î^Þ`?}ÀCÿU›=ÈÀ:Ýeõ'^êÀ<<À%z@éíÞjY@œ©ïR2Ó?Ê ½šTÕ?¥‹"òe¸—?ÞVq[Œî?ÿ[ˆdpm¿î`ýÀµ'?ÕéxÔýó¶¿é#"¿lçà¿âü	Ñ:׿Øã_5o£¿æ}ÆUˏAGNbllCRATES J004901.37+225315.4?ï, Tý;?'È¢«Á?Væ3»mN?S*¨sÞ¿?™‡ó7?'.¢n™)¡?ï‰[(*þ?‹«4úó «?_ç 2}?dn€¼×úç?‰¿3҇¥?‰Q
?ïµ6X+»?¾Ú"ã1?iî©M5á?cÑG™¾JÞ?œ+"H×à?‹p],£C‰?îU–1Ûl?"¿ô3A?g(,ÉéŠ?PÏ!Z׈±?©4ùÔ¬?ƒÕzµO?î@é'²‡¸? o°"E36?k".'U'ß?eM;`>N?ª?JšbTO?ŸÑQ•»?îՃC…ª"?¢ð{üÊ?mhêx"U?z…u¯? Ñ=$Ãc?¡GXÈÝï?햝wŽpµ?¡ÃÞǹ!%?xYlš=q?t%?ÛÌ?±Å}x"Éþ?¡>ð›R<?ë4ð€8Ó?ŸTÓébþ?}Òè­ñoå?q‰ o")ý?°"÷.–?Ÿ€XÔ"C±AGN4FGL J0049.1+4223¿ïö¼5¥ÔÀ4zÅ;ËÀ;*|næg©À<³ÿþR€Ö@ ×âæê…D?üQ¸> NÀ?Ó Iaûc?¿ ãdéº?ï-Ú-Þ_œ@|Eœw?ï¯2Ú˓¿äut¡<¦$¿è$cÂG7Í?"UM[ÊÎg¿á¿m~2µà¿á6ߐðAGNbll3FGL J0049.0+4224GALEXASC J004859.14+422351.4?ïҁ.é¢q?z÷ÊDc߇?3@ô¿ü?,ڝ/•¦(?u‹gEj2›?zpþCŠë?ï¶5míeÁ?]Üï=I?P•Ð8Ëy??WW$—͆B?€_êwÞ¥?€%9ž§ãn?îÅ)ûåŒ?—dm6®?b2g~¼6?o´†ù«?¢ŠF 	?—!ký­~ú?ïv*•?p©"{ß?Qø8MˆÐÈ?;D'ÁQ¯?8¥ôt?o"§9`»?ï±àâ¥Éu?">—E?Am$:|?:¼¶ÁÕ?'põUN©?ƒé˜';ݽ?ïSÝUí-§?"WŒÒãq'?W™\Ô2™ö?aÿXޑ¼?"
¿q{Š"?'éKºðU?î
tzG¼$?žÃE~S0î?h7›õÞO?r,1Ó¶ò­?­Õ>Ÿó±Û?žRBû¤¼è?îR&bD?²³1uaå?efñó@2¯?[""õçbü?©‡*ÃWk?›	b?AGN4FGL J0049.4-5402¿Ù÷47r»'ÀO‹e<š»À:v©ò­1À<®Ð"¢§@Nu*¤n_@j<÷T?Á¨òÒðÓ<?Â.À‡ÅÙ?ý­X"?…@n>§Z¢c¿å3êH֎¿Ü–AöD•[¿áM¦ a4¿áVÊýiͤ¿ã±—¢H"Ä¿ïÿæ4|ßOAGNbcu3FGL J0049.4-5401PMN J0049-5402?ïÜê;ȃ?_Žü'ÈaÔ?SôR"KÍÆ?MÕKÖvF·?iš·½ P?VÀ·ÑÏ&U?ï˞¹`€Á?y#@RÔ®Ü?M¬ª·³éÝ?V¡IÅ~?v{
ÿ¨Zg?uú¡tkü?ïÀ²Y¦\?oyÕêæ?_"L¢?I«²ž#ƒÝ?ˆ«‰ÚTŒÚ?lÞ¤¯…à?ï‡å Íø=?e9Š)×òG?f´ߢë
?H"T_üˆˆ?ˆY°à'Ø?cÁïûXW?ï©F"¹á?xtêé½{P?oÁ?Ô¤ƒ?f ÷¥È
?{˜=0‡'??qš'y*1"?ïc}úñg%?'°·Ê/"??baÙÈ3?oÑ¿?'Dht³†?_é)Ø?ï*S9©?'QäàP‹?oÌ^'-{Ñ?j¹€8¥[?–'nÅ7Ãk?of¤ê?îÐfou®®?'»ó?¹«?znMè?e¾q¨Ùdu?ŸlëðçNÒ?€ÊR³½AGN4FGL J0049.5-4150¿ìؓ¯ACÀRÑÀÁü2À;pÝF—"À<ÛÓÜí@ [k¤hՁ?þìZ{v™?ΒÉ[S7à?¬RÚ?âeIÀé>È?öÿ¶ßO±C¿ïýà5_]^?ﶴÝlØ¿ãN$ É8Ä¿áÅGMƒA¿Âh±Å4}
¿æ%µÁÃY\AGNbcu3FGL J0049.4-4149SUMSS J004938-415140?ï—xm,±Â?''øàÅ?Xf7âzù?&j'~Í?‡Éi•ñ?€'²W}*Ó?ïº
µ2×?ŠÂŒrÈ?TKT‰'†?apuŽÅ|?}çÐ\™öñ?ˆBȒۃW?ïS,‰5?ŽÆžàä?i! ‰;?mÉÆw9?š1y²?'#rX´?ïG"y{i?yªiS‹W?X}r½Ü?HV«Œô-?•‡Ÿ'M?x^ë…cŒ?ïf1¨Y?‰Šþýõ¯?P1c D›?b7—á-?'6Åò•d?ˆ5´Ë÷"?ïSnÞ@Mß?£J5ÿLn?es^í,[?ªT.Úθ?'ã¸W½Á?Ÿÿp§Ì¦ü?î™Å2S?'¼$úYy£?pˆ+îÕe?r'KèÆÞb?¤Rª	¤ã?'_ÁÍ
'?íõ×÷¼ÿ>?"yW'Š?j&d`ª?dÝ¥71š'?¯ j¼^?"k
y¦k+AGN4FGL J0049.6-4500¿æ'ÆnŽÓîÀRo~=ÁÀ:ØúÕS"À<©"3(Ky@NÇÉ-@©WÚ²h?ÇlJ«õ½?®»¬¾åXŠ?㟮†¨Y@Óz›§Ó¿±V
þ'¿æ̬€üꢿç{é»â¿çk|·¸¿ïÿÿ" 5•?èiÇy¦µAGNfsrq3FGL J0050.0-4458PMN J0049-4457?ïäüêå£?\6¾ÿÁÙ	?Høþ6l?F© ÌØ"?dűz‹âL?X.Öbk÷?ï«fˆu/?…¨x];?`úw´Ó@?l#ö8-Ô\?€ç¿ò¿¿º?€•˜dµ!?ïU+Üã×g?"|Z¯Ô•?zéFh	Ͷ?lϗpŠ-?@e†þ'?vÆ(Ûxܕ?ï¸4_Cý?aµbFtð?ZlõÝw?B¦5uÿa<?}^µFæØ?_ø…úã°ô?ïÈ!b6?qyz¯¼xC?Xy2IÄ?^ݜ7›?u¢"¡äðq?màf+0ñí?ï4'¡ã?š…<¹pƒß?m¶—Ì"út?G•¡Wì?•Æ
Ü"?•ß€h!$Þ?îývë;D?‡€¥ÞŸ¨¿?y
bê9?xóp¦8?š̝ðì?ƒ×Žî* ?ïÌ'=«?"Øȏ˜'G?u|ä¦È(?e ¢Gùû?šåöêW¢?ƒ'Õ캸AGN4FGL J0049.7+0237¿ìöÙЍÃðÀNï
å6PÀ8íeéŠsÀ<	"¾pé@° í@P'½´+?¦\‹œ*îk?­ODœù0¿@CjÆGwŽ@þÓºÒ¤R?á' ù	kº¿á'[åY¿ã›.Y¯ž¿¿ák7†
¢¿è'Ì®š¿åÀ×@n/3AGNbll3FGL J0049.7+0237PKS 0047+023?ïñ•uŒbé?KZÞÿü@?-Öut'Ç?"ª{±ï?YFFóæ?HM¸§6?ïêüDÃ?kµçìÛÙ?3*áÀMÝ?E[8NÙm?c¾‡šªš?gÎ÷ïø³?ïµå+à¥ê?t–‡Ò+
?]g"¾ú5?i;Ü1qí?}³©*}Lr?o± »ē?ïäU?!¨ò?JÜ£0h?B¶t`e@Ó?*£ìïÞ?fý#ÓØþ^?H4×øé;?ïÜÊ­|"??bQÖ³ì±8?Aú–øÒÞ?8#±åv·?n¶ÌPKŽ?`Ìús;õn?ïÇN‡—?'†ÚÛu?>0'\–þ?RÃÃJ?zuíš@6?Ôr?ïƒPDûT?Üqš9æ?hL>¡I(?lç¦òçvn?‰ï'\ж?züOìh†?ï¾/Œ÷A?h—¥*øÎG?WH	AÞ·?F."9';$?{sXÏ?e…ÿ	À0"AGN4FGL J0050.0-5736¿À3eÞPÞÀMÁe^(ªCÀ9¾®"½š*À<gKrÅz@k"K÷¥@äwC-|:?°ZöƛZd?f7þ…<Ñ?ÎVüfŒ@¿ü'Çðð¿ÎÑèÀsM*¿å!aña­¿éÅ%nO¿åÀ–'õ¿æQtœŠâ¿ïÿ¢AÞÇ¡AGNfsrq3FGL J0049.8-5737PKS 0047-579?ï÷¼¸é§4?Kïí'j~p?'V+O™#€?*"Rì6Ό?K7'x×ï«?F…³E¼
?ïñä^íSß?b9juºÐJ?%ø›Cbœ?9pü*Ł:?Yx.å¬×?`-cÞUØ?ï³÷•ð?ue79†?Xoˆ½k?bSh{;}?€¬‹åU?r¾ÏV:"k?ïø7¢aFõ?2)qJMH?(ÒH˜;?`׋+â¾?I BD³-v?0C—1Å?ïêŒoZ›?`f¿/]ï'?:.G[õh?2t߉Esç?b.=ä¿Ã1?^Ji§VÐ*?ïÎà'žÊþ?èø¼f»‡?:ö(p¼åï?PO;.òx?vàT0´Hâ?~#/|s?ï~´K?¡Öï°e…?^ˆ.ʱ"?^F¥BÿŠã?ŒõS¢Á?€Œï¤[?ïê»~àtŽ?QíµH´?B_Õ<#Q?1Š*ùªïF?`¬‹ÈÐZÍ?OÃÿkÅa<AGN4FGL J0050.4-0452¿ïÞøڂÿÀPð¼£À9 ܝ$h•À<cæYeÍ@"Eò¨@¯ÁÄ[D?«¿ gå©?±·ðq@­¶åû7@R҄ǥq¿Ïá
?x¿âýW^‹¦'¿æOµë÷ö¿áï åRÖ¿ì—tË"¾¿ä¡Z=c7ÞAGNfsrq3FGL J0050.4-0449PKS 0047-051?ïëG&/>²?TÔÓ¼ã?8Îïê€C?B°-OŽn?aµÿùÆe5?P»%%˜†Å?ïï<ã[/?fï	õˆ?(´Î8o€q?>ݦ8äM?^q0áH«¨?dŒ}îjœ?ï©ü¿Èq7?~^ÈEÕ%z?bp?!åÃ=?px²4XÁ?€äÀN±3T?z*"Uøz?ïôR'Ž)?:ØQ=`RP?*aãl¬y?Eþ¼ÂÈJ?T¯'
#y?8¤ÀoYã
?ïײå¬'ø?e;Ÿl…"?GÿV†)é?9
 Ú9²9?q&ªÄ¦@ÿ?c-;Ø_[g?ïÏÔ뙍?€ÈGh/¥p?BUu^©¿?^ÇPf•Ð?uÊÛ|I&?|xûÙ2¾?ïm2¯¥?†ï<gÕ?j!«
A×p?qÜBìzÆ?Ž4®ôÛ?"ßÙXœ/h?ïáÁ1ýÂÓ?[̎@!'¡?BÞB¨![?8°Rg@f–?i‡=42žx?X.>'›þ@AGN4FGL J0050.7-0929¿ïlÝúØ´ôÀRSÞ¤e¥À8Q'M›À;\ΌÀmC@Q(ÜC?þ¼~ ïÏ0?œ‰8DâT–?¯Ið !Ú,@§¾öJu@?¤T¿?"Ç9¬L­¿×£I›ªjø¿àø%
{"¿ßÛ¿PãG¿âiTWp)^¿åP}'%VÒAGNBLL3FGL J0050.6-0929PKS 0048-09?ïìò€&Æ?R€Ê܂Ûf?3†ýÇL·?&°Ñ$à¬@?`Ïu%ø?Qàve?ïàsο?sØP¸!£?>¿ðõÞý"?Yt±ÔãŒ?k´3åf÷Þ?pÁ;._Oû?™'??"0áéy^Æ?cÛ7i85?rI‹4©?"é1ø?'MœÁ›Y?ïœ] _?m}Ênk?C‡Ë™‹.g?+ðŽ]	Ú?‡°=ž;××?lyÝLÝå_?ïÚa:W"¼?b%âþ•"P?5ÿÛ2øد?,']Ž"d?qoe8u¼?aR®fä:?ï°u^"xS?‡ÆHÔN.3?S…9CMF­?kãS¬½?r0øâ}?…L
­sF?ïŽÛÃÏx?‡Dƒç]?`ÜJHlŽ?jÊ~9$œ?ˆAÈn»–ç?†L'½¢Üe?ï<ÌVo	?ƒ|)]8Ä?R9%üÃÿW?E5dpÖ?—Bê½ ýê?ƒ2+³ŸØAGN4FGL J0051.1-0648¿ïm†½b»PÀQk˜ñÓíRÀ9r}7%À<©&¤¯@€|ªEä@ÜIwBV½?±üàeÛÑø?ÃïÙÂ(¯@ÔçhY…­@Sš±ÇŽ?ïøÇǪN¿á½KÙÅÚ¿ä>Ðñ¼¿ç]žk»¿åv"@Áç¿ïún×S9AGNfsrq3FGL J0051.0-0649PKS 0048-071?ïèÚø'+?V)QÌh0f?FÏæ€Ãk?B;öõ¼9¸?aq
ŒÅ³?Q¡Ájr×d?ïèʟ K?k¨¾8öô?4_ð&£ó?BY••­?d©bïI]œ?hsÍøþÛ?ïŠâEž´z?'õbƈ_ì?p÷|ñ¾®Ý?u2À=E?"Ë°0ù‹á?~•Q*}ùž?ïԃw:Ái?TYț×5Ø?B&åP^?*Ëæ2é7?s{߇­
‹?RÒð'ãž?ïÏ
ÑYZ?kØÞ_â}?[¨ªë
ó
?XÂÁ»µ×?ql²Ð^<?cV0"lü?ïÀSÀz?"²_€q"?K—úd_ýù?gãD:Èúï?|ŒÖÈè&q?Fü
¹h?ï+ՊÞi?àG}íì'??ô€¨®v?ƒDí¾V?'åTƒ™?†Ã«×WìÛ?øû¡C?t¹Å®j¨?X9ØHíãÕ?H"2H8ë9?ŠPƹYÊÄ?slï«jÅ¥AGN4FGL J0051.2-6242?ÉïfˆRÒéÀK6W}•WÀ8¨ìëPE"À;š‡–ü@ÉI®áÂ?ùWêï̓?§ߜ]?¸'\»Aßô@¢:lãX*@hη	?ï1Çù(uj?Ðó=å=ÜÚ¿ÔæФGÈl¿Ók={5«^¿ÛýÕî´~!¿Ý̩܇ÕÍAGNbll3FGL J0051.2-62411RXS J005117.7-624154?ïñ²ò}'Ú?Pˆ¤œ±?7¸8f³ô%?5šDìKP"?V¬Èñ7?JÉ<¦—Î?ï⯂dâ?kå€i8©?;éí¯®´?JºœÇöÔÞ?iÓ@"º?hJä܂I?ï/94î¸õ?'-	—f5*?w.ëY)è?NËVãa?"MSoéœç?G-û‹³?ï¦íS¼&?k3‡–r?Ct?~Í«?/<с?…D·•@	?jJ˜‰â?ïèÿD»"6?\3$ȞÙ6?9vŠÞæ³?4¸0ÁÌê?cÑéÕÙª?Y"ÜèÚe?ï¾+	v©Þ?‹'
%=<?EÞW.}%w?UÆ
³9?~.°7"?€€önn¹?ïI-ùëò?–5à\'ª?{)ú
npÖ?†
ÎWñË?–¬[·7™‡?'˜n‡ƒRÁ?ïPÆ´"×k?€öåÖÝ<Ÿ?Oµ£‹˜ùƒ?@êaäÅI?"é|Ky&è?€Ì§ä$AGN4FGL J0051.5-4220?Ò'55c['ÀR²~|âÀ:Ju†"ÚÀ<vÀ5¯å@3"±¨Y%@rhż7S?ÂítAVâ?Ñô>Á0âK@	æb I@	sM힩y?çÃßoŠ¿å­çχ'0¿êRª\_|g¿îô±ë±¿ï5ç­ù¢ï¿íO›ÿO€òAGNfsrqPKS 0048-427?ïÈ 댴?–¶~–XÓs?g¦¹|]Ր?"ýí}?o¹.W|ξ?nmø:íœe?ïe½g1Åþ?šéíN_z?x!
4$®Ž?Žº=ý1[§?Š€¡»9?‹ð½h^?î':ã´Mƒ?™§×ë{óó?‹ªJŒn¢?Œ°tLd$? Ì1<%/?"¥BS¾lX?ïð(p¯?fjTtñØ?t¾‡k—ô@?[A†£îÀ;?'$»È®à?^Wã©K«?ï˜4uŽ³ž?‡AÜöh?nÞiÚE¥‹?mò"Û\2·?';H5ã?'gdc
?îzö
*GÊ?¯ÊhŠZ?›žgÅÈ2? Ç®ÂÛ
V? é·ÀÖ\^?£-oú¹Å?íÐH´Çó? [ªUì€"?•NaÏã3•?'«h軄•?¨TCÍTõ	?š°–Ru?îÅmSPÆ'?†;**dÇ?ŒÓM©ÝÞ?yôq¢sΪ?™Eëè30?}Ÿú8AGN4FGL J0052.9-6644?Ý)4Á¤÷ÀI28ÅCÀ;DʈNî{À<ô±v/@žë‹©ÁÛ@m‹Ù½v?ĹÚVÎû¿RqÔ®˜"?‹,1"Å«@d3¹jð¿ã_mži3¿Ù(À]ӚǿæøÀ$óª¿ÎïA–Î82¿â ³Ô®Bž¿ÛÖò FAGNbcuPMN J0052-6641?ïæ¢r"?`¤qöÿ±•?3v‡Û?$å1ҍ?fîÉæÚ:W?_Ý
>h·¢?ïՃâù	?pÝ
Åq\æ?AK«®ÄÂ?Gnיü=?s™ò!?mïö;ëÇn?ï~l™¨ª{?z(+¶Ø¢?]îró?`'Ì>á?Œ§eêÎ?xâD7MXR?ïÓ:mAÕk?T,ð‡*ñ?Eñ ''?*¨ÅT,d?s¤•=æ?S¾mìT@?ïÙKÓ?k	£dü¼?>lta?1°ýê‡Ê€?qy¶úƒ?iÅÿoÕ?'¾¯?Žx²³¸¹?PµX±,?]ÌJ$˜?¦¤éÆ ?Œ°øʛ^?ï*,ìÈ×?"ŸÝ÷¼?cß­†Æ=?cþ"'"?˜>l¼ÂK?ƒèì쾋í?ï{³ôh?s(}Q¥À?^œÔÑñ×K?NT|•~z??hd‡,ô?r݁ÌX"¬AGN4FGL J0054.4+8627¿ì«b%Rä˜@7"æŸê%À:ŒAÂB/À<zxQJ@Gœ£º.å@Vº «q?Âàßÿ.žÏ?¾Þ"4³;?ô׿T>E¶@'õf?íâc¢fǵ¿äê>xâ¿ç]?`¾à¿ìiD#‰¿ïÿýaw?ïÿéÅ+ÜAGNbcuWN B0046.2+8611?ï«vT´Ñó?š˜†w'ƒ‡?ZrüDAu?SïˆkÁ<?Ô'¥Ü?š†"ƒ'ä?îû<ÀêZ@?œ]æÕr?…=°ÑF?ˆýÌàH?•ùÞÕa?"{"IHsa?ïw$1Û?€ÞIÓø?mTŽ®¡A?q¦jªD>û?ˆaæÓGàö?{÷`é»Ç?ï!=Íôr·?w̽öT·f?Ø@~¹Y)?eCߺ¥Ô?'ì%þMjš?r-CS=Ÿ?ÖC.?"Æ^×oÌ?qù¢ݙ?i?N#Ãaf?'Í­MM·?'µæܹn?íQV²c	?µäo…ª?—ùÁ~cS?žÝÇ?¯`—ÿÂkÁ?°øS¶8ö<?îâK絆?¿b¡¢â?€œæZ[xô?€a—›ÑÐí?›hÔvs×?‰Ú¸ú??ìÇ;±â?œ¯DÎ&™? Jä›C¿}?‹«µ9®¤?± ´×ªÏ·?"žvâ°DôAGN4FGL J0054.7-2455¿ê#óPÞلÀU놘5ŒÀ9igH
¶À;õ8Lw§×@ %"O…y?úîuÿ`Ð?±YéA¢?³¨Ö£eJ]@-J¡!@§
fÅÜÄ¿æi'z™#¿Ú¡5Ú­` ¿ÙWQ †¾¿Ö4;‹ú¿Ø¦•€…K"¿ÞAÒ½ý|AGNbll3FGL J0054.8-2455FRBA J0054-2455?â\ÏÂܚ0?אv´žG?JwÐr7?W<š'h?Û9$'=Ž?ד¦ö¤b?íîýZ+?ÁY®mÍI0?b™Šx:š?w·§ hÉÏ?¯æ'·%…F?Á qî–?ë	È£"?¼éÇÕþ5?Zúô&|ÇI?LYа'a?Ùâ÷}òÁ?¼ñ÷ØØãu?î–Þèœû¾?'N3 Š*c?]zß%´)q?E-9ö<"?¥¦:xãá?ôÖÚ)p)?㽨˜¡2P?Ó­k .€"?u‡:¯n"?wŸá!6.?Ø.'äՓV?ӅÂu0?ì	åÁ‡Á¢?Í®jó$5¦?mºek
šë?€§7ˆ»?¾ÂþËU1?Ív½¬Hrà?ëCkG ÐÛ?¸É°ùü<?keÍ(Û?g[:ЖÉñ?"»¯ Çÿ?¸Õ$YšˆÔ?ìƄŒþ;ì?šªÙj¼x?nû×-L4#?`{µß?¸Óüß²€?š!…"ù†AGN4FGL J0054.8-1954¿í+¶F©ÀT¯ƒÏ,ù]À;V¢¤V§À<³6z—@·"6Æf@ÛeìÃã?Ë8àä›v?²'xÛJ?çy>@Øb@q¦KÝ«?ïú;Àu{'¿áZ³À6fn¿åôIÔ_h¿ã=ˆÁÛC¿êÃ
¬+l•¿ïàbb ´AGNbcuTXS 0052-201?ïèÍx»Ÿö?V‹gnýxa?7ˆUGÃgH?)Q'\J?dA|W'ˆ‡?Tíâp%?ïÇ8ñO¨?zøÀTÉ!ô?OvFTzÕq?VÔß²Vû¢?xu3Öª?vѹûtº?ïŽÅ‰Ÿã?}8Æ¿pYŒ?_ö>t}ªú?c&¹GŸÔÚ?ˆOò§9í?{D-輇?︵Œ¥{‹?`êĞóÓ#?G«ý†Oá?1$8‡¼?€WÝsî2?`ÉeÔ6×?ïÂÙ¨í
?p{
'àã"?K靬aÁ?@Ì0˜×ù?{r߂ÉSà?n徛¾°R?ïo3iŽå?"ԑHYŽ?ZFâxiÍì?k½¼¤æž?Œ[VÒo…?':/䏰8?ïBÀú†™b?…³@Hj^
?fÐý/P?i=û|¥O€?"ÍÁ^¯¼?ƒ°xÙߝ?ï È«´?}®†WžÖ?`*‡T%þ¹?P`'‡SBò?š–•ø4¾?Z¸v@AGN4FGL J0055.1-1219?æ¢RÄYFÿÀRʯáÚ{À9ýÜ-'àBÀ<m×ΈŽ¯@¼p¬'ð@
'¤Òh?¹ãD![ß?ÀÞÏ-Ðã@F{¢7ÍÍ@2"iY
?ïç«?´Jö¿ÝA"ßþÙ¿ã—všÙ5¿åüŸù/+¿ëC0×8`š¿ïÿÒkÀAGNbcu3FGL J0055.2-1213TXS 0052-125?ïæÖ7ð˜?WOÊáâ÷?B•…˜Ø³?6l!u/€?d"…ÞYÙ?T"›Ýúó*?ïëynø?l{ ™lêæ?1Àaúk‡?DƒwEÀ)T?bc•×?h‰@"pi?ï +Pˆ%?za±Ñ>æŒ?iÊâ\™š?pìuoe?'sLOÒ7?sÞî¡T—;?ïçÚ;›=?G#ß®¾r?CáÕ§Ûû?*ÿ¥&_ÇP?c-|I+‰ó?EÃöµö!?ïNJ ­_?lÛߞex+?]àîœõ'?TG-ŒR?qo't'?gÙMº¤%?ïÃ	Í粊?®Ýéù°?A?ƒº^ª5?Rü)ɉw?|S(ŠÒp??€jlË$j?ïZŠ×x¼?†ÙéöXŒ?x<()à¾7?}¢°Fݟ??6'É?­.
M5'?ïÂc–
¯&?d	ÍnhT†?Xžš!6V?EÙLÉ]û!?x¦Ž\ím?b46[ÒAGN4FGL J0056.3-0935?Ò0WjcåÇÀR¸ºÇËÀ9}îþOü˜À<÷FóÚX@ù¹î"ÝÑ?ýÑ–^{¶?°_˜kòˆ?|OðŸ%?ÏÝ=ëô@÷ü\‡jm¿ë' À¿Î7¿ÓƼgyâ¿àÔÀ·Ô£¿Ú:@m®YD¿ây…'`lý¿£\»~óAGNbll3FGL J0056.3-0935TXS 0053-098?ïô`.éÍd?JÈLpx[§?!ºé0äÿ3?Þ¹ ,Êã?UDŽüå?H³òâ§Q?ïí—?¼?gšÀoTç?*_
1Ý?:ü´â'?`ÂÇïÒ
9?e'9Iá—(?吝ŽÌ"¡?{IÒ3ç?T®%H`*[?T(Ēg0q?ƒ~לïšn?zàE⤰½?ï­g0_?bS­f'Ò?AæC<u1j?)2†â6?ƒ‡·ø\ü
?a'ïF'"?ïè¶
Ï¢ü?\¡)•r?4iHIï?*ވˆ¢$Ž?d¼ÌáS­?ZJi*EØ?ïÂø³îÚ?€c	ŽðÛa??_µ³?Qà…¿Y¶?|"÷¾ôå?~ø¿!œž?ïmmT¨_?ƒ ÍªÂ/Á?aòön»?jãGq|?2©Qq?';…ŸŒ+Ù?ïGñq…?qÇ5è¨ù?SÑ\g€µý?Coék¡"?•ÄLJÍñ
?~R ·üAGN4FGL J0056.4-2118¿çñKJ'[žÀUþ!ÙnœÀ9Œ Á@§À;ý˜K$Â@"żãÊ?û·ü«·©O?³+»Æû}?¿›?¡€˜Â@Œ˜¼úDz@	Ê'§…?ïÒ"4ÕË¿Á9‡ ÄÌ¿Û<á²·ù¿ÕŒò3Ž£¿áV:¿n•_¿ìcxt…äAGNbll3FGL J0056.3-2116PMN J0056-2117?ïðJÛÜà?O˂Îêœá?A÷…R"Ù<??$þXê'?Vp3¨Ó»*?FlyÞÈD?ï4?®é?׶?jì\ÜÐ×?…¥™Øá?–J¯:f?ª"Ì68œ
?·?ˆµ¨g"Å?q|8´IAÁ?{"¤]\~?‡:_0îސ?ƒÑm¦ºª?î—þê+Wr?ƒõ&_ö—Å?jK¢™á%¿?ROÖA°"?¤ÛW0ߎ?ƒ,bž)O?ïÚÅ5 ?³?h<Ñ®::æ?Z
#Ãf•?Uã÷'vF?h48½ò$?`$‹bÏ?î²  %?®ÉOÝÁ}?y¡vpi[y?"BgX©ºN?¡¡Ï"¾¼?ªÛ1ÔäHi?ïÍk"_?"Wr½?"ˆìœL±œ?ˆG—`‡¾Ì?'ûpgW?‹8j2Vr?í	&õ5]?šÏýå»´‹?xyK.Ü`?hw/æ
lÐ?¶/3 ˆ¤"?š…žÛí¥AGN4FGL J0056.5-3936¿ïÝ?¶¤AhÀS^/@_k À<6ë!LÀ=¬Âý@2@½}9;¶@%1ÛD^Õ?ܪâ`?ï«W½V@)x]@°Ac¢'»¿ïûvÞ®¡"?ïÿ™=SG¦¿ÄOF,Š¿ãuC
›Éö¿ïÿ¾AÏ?Øх™1"ÎAGNbcuNVSS J005620-394144?énáÛÓ?ÈM·gy¥¢?ÂxgŸ	×?ÆÖÉ)C	.?­'ušùÐm?³È¥N\?ì<–ýÄ!¿?¬WKì<ª?°vù°«e?¹Œl4†šc?«HœÄúÎñ?°‰ã
@?è7##šÜ?±
héÂ_?À©q2È)O?«‰¤zm`?¼ôùRր?¦!n\Y?핃àÓG™?›r)'9?«"e0³Ž?•QÉK4?–(¹ŒÈ¾?‰Îí5
ƒ?ç¸1úpko?Ȳs`±û?ÅÏ·ÁU}é?Å4 hP=?¶Ÿ¨Úµ?¶!ÕUǾ?薫cN6¢?ȈmWoÈ?¿È©°Ã?Áßè_œÀ?»û5s‡ë?º×ó\µ<?åœ8.^{û?µ"/îÁO|?ÃHI"bfì?°îšÓmŠ?ÆFÕ²#©(?¬ÔרàîÊ?é,›W<…u?²œo¡scÂ?À½nöWà'?®¬ënCƒ?µ GXþµ?©ôè‹;ªAGN4FGL J0056.6-4452¿¹ÂN<РÀRg ù	lÀ;/­¯ÑƒÀ<ÆuŽøUè@ˆfed³´@½ãÖÕ?Н™šäó?Çj½m^R?ò‡'Ñ(| @"'R"aª?ïþ·€ŠT¿á3A
ŒJü¿á*XÎÎ.Í¿ë)«Êô…x¿ÙccGP!¿ïÿQ"W6AGNbcuPKS 0054-451?ï"æ,«jä?«@Vpۃ?vâÒàæ?«,J~ÜÝo?ƒUjjTü?~{ºì¾š[?ï³p0¶ù?'¡,]õŠK?^¦ÑDé…?f*Ð6"d?~ìÞ+Ä$ð?}%ðÄ=?îïzàØ?‹žò¶û±?€a©ÙþÈ?äD"¯,?™ýŸÕ'L;?ˆt"óî?ïwl»•þ?lÎϟ"º&?[ùԂyȓ?Fn9Û½Ÿ±?Ž¥–êgi?k(Û^g–Ì?ï(Ù[.,—?'bkiŒ^é?fñì8¼?fí@WÚl©?˜—â¨?Å"Ú+¢?ïV$ÏÃ!?žÌÃëç? ?p_$Ïq?}À"Ðr ì?˜}r7#.Ž?šo%"´?î)RÀ—?—A'Þ-Ê?ŠÙÐê‰cP?†È‡;õ®Ö?¦¹ 1¹?"œ@zßé6?îhðN²»?‰>Q*‡@?n*ž9;Šñ?bâÐf¬©¹?§ŽQ0Ý'?ˆµ»óºÖAGN4FGL J0056.6-5317?í3[½sœ
ÀOèMüãÀ:ïiÓÀ<ÔüA.žy@õPŠ\õ?ÿÖt|?Íü´Ük%h?É-´C>??ûG
‹ýá@n³}ÆTc?î9•"zœ¿á,c5Y~!¿â²Ÿúܪ¿Þts®M†¿æ̚wåê«¿ïûç6Û^`AGNbcuCRATES J005630.93-531931.5?ïø¦XUæ?N§Œ…6ƞ?(I0àµã?)ãƄ›•F?G_ÍGq(?Hˆˆ:›b?ïèw:t.?iËRIÞü;?0Ó	ÐTëæ?<퐃Žj?endZDN?g<:ÐÙÊS?ï®{gn=?p ¥TøO¾?ZLQh³?`¶«ÔSÜ¥?›üð?kD›XÀc?ïÛ'AýW?NKÑuÊ?ECvœqj?(%ЯÇ>†?o–­M Z?L8æÏ{?ïï@¾û?^""jR6?> ¨Ṽ?<é'ñíø?YöWºmûä?X=†mÌÇþ?︍‰&@?'cg6қ_?C/ê9Sb›?RJþoËÙ¢?€©Ÿ3ú/?Wõ…IÌ?ïvõ÷'FÛ?{YæK/?dËögí¦i?lQÅ‡ªu?"Šò??{<°³J¯?句«'y÷?j¢#É`×?SÀ´F^U@?BòªÕ?"f>…Ç3Â?iåø¹Úí¥AGN4FGL J0056.8+1626?äȱÚ$›ÀG5HUÚ'(À:úÀ%zÀ<ŽOÙ\'@Z%"ü|?ýÔ§Ý);c?×spºþI?ÍËù'ɝ˜?ó«¿¼CÎ@Ÿ''À1?ïԘ"¡¸¿è¸¸G¿ã3Ìý¿Õý-};¿õ¿êÐà"&þ¿ïþÈþ3:AGNbllTXS 0054+161?ìêÆGwÖ?Ê OI?^H'(Ì?SGãX|[W?¸0­Â§w+?Ê-æDd€U?ï´_ürŠj?wû%L®?S?߈K'?V}Ézl?€€õ²?tïëY€÷?ï.×÷MSñ?‡'ºØKx?wVîôFè¸?{i¦€ÀP?"OE]cO´?ƒÀìp‹k?ïÞþÜ)?q³êN¥?f*ÓYI•?IÊc@í/?™¾ÅÁù[·?q<»Cμ?î€õgu?±îÃ&6Ê?rd©ê ûi?oõ™çsŸf?¥¤K*dœ?±yžu51?ï2… :Þ?'üÌVË·Ñ?b€‰[•žT?nVL9؜?—Wž**©?&|Šwå*?î±ç‹¿ç6?×hQæ>?›S¬õî?~""{/Î? îÑ›œ?Œ°²uô/?íî7ÓMfÝ?Œ˜Ÿ$œ7F?pLxT?b±nu‡7?¯yG"^?Œm)gò€AGN4FGL J0057.0+4101¿œ¥È»•ùÄÀ5×qûÅޜÀ;RÏè
?õÀ<Å ªšrÝ@ '¶%–h?þöêB(™|?ÎxADÃÔV?È#ýu·O?ö'/ðˆ"¸@²æ˜>%¿ìuŽŒö(¿ïþÂé<+?ïú½ÖÄ.¿çÖBL*Ñ¿Ñ;\øSŽ¿ïÿŸ‡ð#êAGNbcu87GB 005415.3+404404?ï±Yù4xœ?‰.¾'š-?QP^¥Ça=?JúÒjÓs?uÏbšÔ?ˆþ\œ "?ï»ç¿8Üã?~õ]öd{?Pñ;Éß!ƒ?\n"h¶?}ÏÑT=i?y‰gÉA®?îÎ=˜@(?'½…©o?däá"½—Â?e¡ˆþÔ¢?¡Íá£2D'?'}èüå¯?ïq:̞mƒ?t2Y•YÛI?E$֝x=C?<]èZË<O?'/´x?sÉkì|³a?ï4?Žò?•n»•/7?d~B\3?^q÷jåd?–èWƒ#ÕU?"³–oîzr?ïK|õŸ?"·j¤‰mÅ?a¾RM
7ý?pŠ(‹#?"VSÇóâ?'oz¢¨?íê
÷u©?šì³&Æ?oc7z3£?re.ü?r±?¯i[«z×2?šuщ¥$?î{¾­­ÖE?'b¶¥æPy?RäcôÉy‡?T5wäóŸ?§¬òwã?'$³â}AGN4FGL J0057.3+2216?ã;e¿ÞŽÀDIúÁҝÇÀ;®ÈÕÇGÀ<¥h[3,@¬ñ\y'´@G•övêB?Ђ§z,ìÈ?ˑb"së?øŽv pMp@‹ND†˜?ç{âN"8¿Ñ!Åâø³0¿ÛK·c"ä¿æ#ª"" [¿çñž¨ÍD¿ïøuÈ9pAGNbcu87GB 005452.5+220227?ïƃ?4{?v"'#¨?QK€ê"`?N4h©Ž.Ò?xk êÍv?s0úÓT(1?§8=´?zø5óå:?XÔr1š‡£?X¸Â%Vï?…:‡æ=â?w´z¿ïY?ï`Šoì2T?|h·ρ?mÞÿÙ¯SS?j-D~ۍe?2Ò˜p?w¹D¥–?ïFj@¡Áí?m€â±ÅP?lS¯L?J†Êu;—?"°t®Qg?l)u¯ƒŠ"?ï"Ïv¨Ü?x²ËCàª?aôgêÀ?U^FúÚõ?†›ü¬•H?uïIjì?îâþ»ÃvH?–'©ª›ï?lü£

•!?sSºX&?Ù? J´!1?"ð­"²°ë?îét8¦T?ˆ/R
:?}2¥VT¸!?yâس#4?›"Ô†A²"?'€Räï?î3ÛÑÄС?ˆbÉ!<RÑ?yZŠÓÔæ?d¢…tœ&?©–êŽdîR?‡È…ìÃAGN4FGL J0057.7+3023?Ü­eqáUÀ@:2 f<uÀ:]á‰ó3iÀ<qƲ˜¬@à[À6ã@/¿üñý?ºW¬5Ów¿ù/£©	q?áájžYqá@h…2`z?ïÞßY—K¿ÚßùD¤õ˜¿ç2Ö·1Z¿â·U¼®¿å"÷¡aº¿ì\8åú›<AGNrdgNGC 315?ï¸xÕ²W3?t¯¹P%€?LTS_D†9?7ýÍ`ì°4?€…n¬Â?sþ?çó®?ﵝ@m-€?wâßTÚ
?Ql6ÇZ?Tñ!˜9à?€k)<µ?tÍ
§Ô;?ïP¥«ºrF?	¶Æ{Óú?png†]è?mL€IøK?'éîñÏÁ?}to÷0cû?ï'$*?daû"˜¬Å?püØõǂ?OD'5•má?†ýŠÎ³Sj?`È»k¶'e?ï3ʪÍ?%
ϲrh?cÁ­Ü]Ê?Rµ7áîô÷?—&±"Tò?8XCàjé?ï¶§û»?—üT?e[‡ž?qË´č?›ÅrjŸ"Ö?•¹ó"$E?î¤ÍEÝHµ?'"g1"µÆ?Ï.g£¨"?z–|qR?¡¹EØè"?	€oA¥i?tbõ»?€rɎèZY?‡Q0ŒIUÞ?l¦féÂ?ž`¹/4k°?{2‰~¿.ÇAGN4FGL J0058.0-0539¿ÆÉ'?f{ÀQ1&éyÀ9àL'ÿzÀ<>$ìz@Ž¶çˆ:@Œ_|gY«?µ¹f"‡Ý?š%™¼Úç?å·;"@ßÅÍÕ¿¼o¿*¢Àà¿äu0cu^¿çéâ‡I5¿àïâEÚÕ¤¿ð?ïÿÿ" 5•AGNfsrq3FGL J0057.9-0542PKS 0055-059?ïñäÞ*\?d¡ó&ȇ?7ý`L ´l?1ºz÷1Ï?V6ë²<¾ý?doØZ!?ïêԐD"?k?mµÜa"?1Ê,°®ÿ?AŠRé˜?bò*9òb†?htÍ$À£?ï¹P9•?váSôŸ%×?f'ðïXý?rñ8I`?xkQ´´ò?ky-'QWQ?ïòg"É?@Z²ZIÆ?'Õ*E¤&?‡=G[R?XéI¾è™?>´Áú ?ï聶ÎÞ ?dcHò\³?H³Rùä?GÑaúdܦ?aQtV³ÿÃ?b\ã obï?ïˆÂ"m?ƒùí]Ž@?CôÓïc'?VȱEn|?|=V÷""?pãÝRˆ?ïu÷;Ð?€‡Jœ¼OÛ?n´…úɓì?u(?"u—ûïƒ?ufõsZMÓ?ïփÿËÊ?`–‡Š³*Å?C@Þ`êSh?6~µoÿ?rUäQxÙ?^è6ý'{AGN4FGL J0058.0-3233?앒Ïâ>ÀU>úç'À9?ÊKM
À;ý±Ù+á@›4
MÆ\?þ§"Ô@^•?±MŸ^ï=?ÃüiÈp@ÒàýÜ9Q@Ãö9'­š?Ì♨28·¿ÚtØdZ…¿ß´© !óñ¿â—¤—#"¿å_‡dU¿ídÂw^[AGNbll3FGL J0058.0-3233PKS 0055-328?ïì†x?Y¡Àÿîô?L#5Ÿ
ÑP?F-ë,nk?YÄ@ë¼Sé?Pƃp,×?ï²:É:Ø)?"i…ôƒò?W9YޅÁQ?t&â³bZ?€Š"dK1–?gŸÃ̕g?îÊôôç?›â½Dnš?–Ô`‡,Ä)?•ãÀP´ð¯?šæ|Ñ?Ž–Ëy‰°x?ïŽ;Q1Be?gÛ
zbà?\?x±"¬T?D¢C|°?ˆé<¢¦;F?eò
Q]?￈šTÞ?urâÜ@ü?e(}8l-}?a禤8hÛ?u§t'äp?nƒB¨Æ^?ï/]ý‡?ªN€öÈdV?qî
?"Ê?‰?QÔ§ðF?•£TÕۙb?§Xã)²5Z?îåz›?œ¥@]fƒ?•—'E?"8!,æâ?˜Ð¹@}ôx?'óâíðÄ?ïüè.¹7?'<ËuÿG‰?j÷>C¿=ß?ZE,èêÝS?›á{9ðS?n/¹N;AGN4FGL J0058.3+1723?í‰ëÀÀF¹àÞ҈ÎÀ;ײˆä@À<àòŠÌw<@"\øžC"?ö¬ôI:Ü?ÙWM¤xšÆ?ҏ4¹¿ª?ûG&Ɖ½@1ƒ°¤"¿ÎЈgB.¿ï¼ÚF2y?ÄO{τ7?ÛbY&D¿ÕäŒq'êS¿Ó]$É8AGNbllRX J00582+1723?ï¾ô_ÁdA?vbEÙù½
?Df¯¿ÿ<"?:BØ<Çì?}øúIª€?u¾…áq?律‰½ó/?'í`Áºãª?\Ÿ-ŸÐáI?jêôL9?'…÷ÚÑJ?}-ŽQ¾˜ê?î¨ÉÓHæ?"úCM‰?fŽ&SÈ¨?kŠúÕ~¹"?¤
€kÞ?"Yl‹w¥?ï51¯=?}Ú
Ž?AËßF*3¹?3tر®9?˜Íºè± E?|Ú|Ͻ¤²?ïw¼ï"üÉ?‹Û$–qÍÌ?S=(•Ð€C?IÞ¶`@?©ÈMÊ?Šô9Éw$?ï0C8Ü6ï?"¬&ÐSˆ÷?dmaRæaà?tâëÞ
#˜?—iìÀ£—Ì?'.Ý8)è?íŠdÑÂÞ?¡~˜ìóŸ?i
õß»?qe`ò©V?²äƒáÚ!µ?¡C»;†½?íµd
Ï)&?›ñFZ«'Ø?Q£0神8?QÇ(Pþä?²RÎxi?›Þ¤zC*AGN4FGL J0058.4+3315?ßóTïN4ŸÀ=™-ÛÛ]‰À:ŸZ±&~À<ƒ3ÆÖé†@¬nëÆ>@iød*L?Ťò}¶d+? zƒB®êþ?Ö¤b‰·ú@M™»ÓU¿ÚWvÿÄ^¿êxbý¦3†¿Ü›aÅ¿ã½#â]¿æÖ©ZýV¿ïÿ¼ä!}(AGNfsrq3FGL J0058.3+3315MG3 J005830+3311?ïôcüÌ\?JÊÂe#ú?!"7'ñéZ?þV«u¯w?U¿•KÀ?IZ±Hý`?ïëÆn}¥â?i
¡A2?'RT‡&Ž?8KX‹°¿?bÄl½r?gˆ°Öà–•?ï'γÏ?oœ[p?Yþ"9m<ú?e>³v9ð?ˆyÃ÷wW?€Y>ZµÄ?ï÷'´?Z?0fWÂ|ˆ?³Æ7ê{Ì>öÛá;'§°?P·ŸËV9ü?/̾ À¸?ïßBI-Æ?kqÛï½X4?21Þ§2ª?(Éø¡"Ò?n|eŒ3?j¿-'ƒœ?ï½³ß@?"˜òý#†â?<{Œc¬j'?R.~#ÄC?«F}…l\?ƒ5Ú'hÛ?ï:D¼iõ‰?g«Œ•?bèԖJÿ¶?n†.,Œ³?–ZM㿀Õ?Ž	ýL¦Z?ïèð7œ4»?Q²qýz?#'ÎÕìˆ?}ÒªŸfç?e֛†ˆ?Q?"¬q±AGN4FGL J0058.6-1140¿èÊ5ùêšÇÀRiÂ;ySÀ;Tük 	‹À<¶g÷`N@¡'ðµµ.@Êyžø?Äqw¼zL¿£ð ¢³"ã?۝i?þÁ¶é¶'y?ï¹c<{¿ç³ì+7¿ËÑþdõM¿èõ¿Ÿ½ 	¿ÕAé"h"ú¿ßÒ=ºu²4AGNbcuNVSS J005832-114050?ï°õÂÔY?r5<äi!?Còóþuá=?3Jÿ]8Ú?'ƒ`³]‡?qÈÖe­Nò?﹉傷f?ƒe±1Q5ò?ZA§&4q?fTØY¨ÔÔ?|ª£V*´Ø?}°çÇ œ?ïJåV†ty?ƒP˜?g¸Ù þ¼V?e²Íw¸?"¬9úåž\?ˆJEÚ8ö?ï0Éû"Ï?w™^Ÿ>gx?O%9âäíÜ?>!ÿN•<?˜íµdþ¥?w€ß֘<G?ïeúªD{t?‡i*¥•Ý??U͎¬iJ?HéÏöá÷?'ðÛÆô?†Ñ~!,?ïX½Ãl¥?–ÛÝø|u?dÇø³ú¨±?sô/‡a?'OH‰þéL?"Ré±N?dš´L?`"ÇÝ+?q`.F—òƒ?k¢Y®2ˆ?¢ÚSé¤-x?ŽÜ´Ñwd7?íV±G`;Õ?˜ÖÒ›"?cn«d¶M°?ZoñÕoފ?´¯hm˜-?˜(X{ю|AGN4FGL J0059.2+0006?«žØu[þ'ÀOXn¹ªÀ:Ôf_°iÀÀ<g[±×~@ðü@\†Ô?Æ3°†›;?!ßÑa\w?•GÒ¸°Fk@Ê}ª{¿ïûSþ"Õ½?ï"'úñ¿èýk@íù¿Üo<"ððÿàÄŠ]¼t¿ïÿ·¼]êAGNfsrq3FGL J0059.6+0003PKS 0056-00?ïÈV£¶‡?q>x²Ø}°?Dæ5w7¤!?9óbtïý€?y86yx	Ò?pxnÍz^ ?ïêCL¨F¨?hžÂ¶9²?0Ց¥+œ?Bõ´ô"ý?c¢	¦Û?e†¬|'G\?ïQÌðóë?'+1&~œü?hÕ œÅU…?jTOBK?'«ØV/ñç?€P
ž?ïÅN~_¤?ZoÜè|µ?I
»¼8ä?2
YÜQ?zU¡m[¡´?X¬fbÐþ·?ï¥Wל"z?yÂœÄû?TàÌԜ‰j?H­åˆ™ts?"
ð|Te?xa'ÀW5«?ï¯ÜBê}?"þ|,ÙJ?JçZ2Öh?h‰"BkL?'gщFõ?''´Ö .?îÍÖÒ¨?‹lª¡tq{?rïtD³¬?q?TÇ°–? Ä¾jÀA?ˆÂ%m¼ŠÏ?ïr)#v
	?v#žó±?_F3•?PÝJ£\?"¶¼Ñ=[?tzÂjKÊAGN4FGL J0059.3-0152¿Ôÿ§aû•ÀP+±mÀ: ö|ÉÀ<om"BJ'@!1‹¾9·?úJ"H)d}?ÉT™_b@?À:îéWG?öäŒ×ê7@w¤!¸?ïNëUN.¿Úb/ »è¿ëM&ßgÚ?Ù>&@Üi"¿Þ‡j'̔¿âqÐý³õeAGNbll3FGL J0059.2-0152RX J0059.3-0150?徭*¸?€úã9	‡?C²hó¶|ô?@‡&^?"Dx iTG?/æFvT?ïÒcÛ=J?u£®Éi.…?C÷Ž¾à€'?Mu¢§?tO‰²ö&Ø?rý½JÅÁV?sW?ñž@©?aÞŠy­Î?ULípV?™ò+¸ðt?Œ¢€=À?îòÕ\_É·?ÿ¬‹	Æ?bÓdðˆQg?Q"gb6Ä?ŸJçÚÅ2ú? gÕV}?ïLý~gÜU?'jiZ€ŒÕ?YU¹—$B)?W…$Õ,?"Êô õZ??'˜sÓ1h?ïf;À—Ø?–ž¸Hx˜?W±aAÒs?f]´«ÀÑ?Œ°D鯷?‹ùvžÎÕ?îZ5^9Nß?–ú¼IFðÕ?j·#Àª)?gvñc—?¨±7Ý÷Hu?–M™iù£?í(¿`lk'?ž[êc?þ8?|+ױƣË?y°y—2?´÷GpxŽ?µraè:AGN4FGL J0059.5-3512¿åÄHwúÏÀTnñVIÀ;-‡˜æsÀ<×hL´@ '¡R Œ?øàLÜQ¥?ÔÓ)=+Ç?Ú·æ@'?®@ºQÎ_@'.¦[žâ?Þ÷~°4;¿äRKý."h¿Çáä÷eý‹¿ÕÝmCzS-¿à_'¡Û\ˆ¿ïüjÿÓ4pAGNbll1RXS J005932.3-351049?ïÜÝjm Ü?h-¯³Zä"?GX`|â¿?@ËF uä?mL}±¯ƒœ?e®rœ½)?ï²i8¶•?€Ó3¢{‹Ù?X¾‡ÑLc³?`†Z}!?€Má¦îM?|=ÙB'¡?ïR'C??†±O~ÿu¨?p¨¯«®u?qʃí{Ð?'ƒ«°B^'?'ØÁjH"3?ï¨4´_?sè°¸W?[0xz
ƒ?DíñCåôª?šê	ò½ºE?sD,Ó¤?ï»ýî>×?p6VúEÕo?]‰$‡éð?RŠBÏãv•?zž¿¢²'÷?kÔÿV¥éµ?ïC¡òûØ?š°Ï§XÛ?pçÄömÈÄ?'˜‹?"Mº{šÜ?'t6	†¤e?îêûŒ™£?'ÑðY6+?u·""h=Ú?x7lµGæ?2¾‰·%%?Ž
^0Žz?í³BçJg?}ØRNòÐ?dêXàT0´?Z3O-|Ê]?±¾•þ¡´…?B'6¹AGN4FGL J0059.5-3338?éþ¢·œÜ<ÀTÐwpyåŸÀ:îßDž•'À<}þæ$Œ§@ÀQ>@s³{j?Ä(3e]&ø¿Jèåë‰?Å|ÔýGéÏ@8WÁÝÛ?ï€wSôsÛ¿çՊv'•¿éÈ	ïm¿å
@Zc"å¿îâæů¢¿íå¿ý±q'AGNfsrqPKS B0057-338?ïåK‹ïŒë?_!*ڍ—?Qx;\kˉ?H×¹¦@3ò?aøVVv´?Y•¹'>Ñ?ïÅø¹©sE?…<ö1¶?RèRb™s?jÂÇ9â\?xIŽª­\'?™ÉÄG?ïq×ÑDE?}þOÅEà?d/Â
a?_î0°.)?Ž~MÍc+¼?|Š?ÎÒ?ïÐõ幜ˆ?W Y6?Qƒ9Ç&8²?;=èèTD?s$>•;aè?UIv·.f?ïÕÅk¦ä}?juwÒ§³µ?`©¯MúK˜?X¿4B°´?iå4\†ô?dªüXÛ­H?ïsÁÿFû?"ýe¢Å]?\ØE­Z÷?m.FE{ä?tw'4у?'#¦ns?ï(jò'?‹{½õö:?o»;Ž¤-©?iµû€è"j?›ã‹+÷èu?‰GӔ—E9?ïv
Ö@¡?u­Ê.´Ñ?kªíæ¸/V?[oÔhyd?‹'{Ý?s¬O™HYAGN4FGL J0100.3+0745?Û&™žïfLÀK…}™ˆÓÀ9À~à°¯À;¸ ؽ›×@~DzƒSÝ?úñ`åóå@?°'IïgÂ?Ãahz½¶Y@Y…ðoiD@
õöA:\ó?ïãqߖS¿¼j»_¼þù¿Ôþwštá¿Øót ¹3¿áÏû'½¿ëÝ­Å ‰AGNbll3FGL J0100.2+0745GB6 J0100+0745?ïßSƒpôp?dP6äî*?]Ûn±$®î?[
¼à†>#?a¾Å	`¸?T§|‡KJ?ï—0ÙÅ6^?š¶My¸*?c½œ5.Ñ?t'Ž‡ˆ?…nÚ–˜Ù?™tÊ}TR?•g'N?™Ì+Ü	¨6?•¢æ–ÄÊl?"ybyp?"kƸæ¯Û?•%ْ߿?î9d`Zf\?‹Gs@›Nñ?w'xÈ[?]m">õÓf?©"ÊÞÍì?Š"Ž'5?ï¨QlaÜ?z¼É>3ם?t[¶ j¸?puÌ
E+?w£ ÀÁ²?n5ê®KÄ?ïU¶¸/Ô?£¸Xʽ?z°'µ¨A?'«Âöf!"?˜I?5¶Js?˜g¦ØF}"?îtx—WÂ? ¾"&OÝÔ?˜?]~E?—yæÖ N"?™1Ò¼Ïy?"ÛLJ+?ìÆ"¬þY?Ÿöº'HØ°?"–'Uî?qàΌÂ}?¹nXˆ X7?Ÿ¹³éAGN4FGL J0101.0-0059¿íû͍´UÀOáXâe,À:봙Р>À<[‹)"N@•)œ±|@mFTx'?Çö¬m±´¿"o:Æy³?¿D"Wá@àG
€Œ'?ïQSµø ¿ìŠ…à)Jý¿âÛȳb˜|¿ß㲁òÞÚ¿çï\¿Hª¿¿ïþÛ<ÒfAGNbllNVSS J010058-005547?ï|Ø©W…V?šë–µO?Jv^CÚ8?<ZQ+é'à?"o¸ìèn?šÚƵ†Š?ïÄN8º?z¥nqG?R97þwÖX?Xè̏:?yJ•ùôœ£?v=¶n7}\?ï1Oj)?…å2ˆä Ä?cdÙ1Ø¿È?dX‹)Ö'?—pð[{?…W™ö´óT?ïS|§£ûü?qý–Œ%•?SþÓ(™m?8$"Nº\?"PŠÒ™yë?q¬'ä{1%?îugÍ2'?¦q!~ ‡?s¶ÏØÃl¦?ž
ÜÃ^à?¦2©.8×Ë? õ·rÊë?ï`½µW»(?"¼Ækõ÷‡?_9ž×N
?i²áKWiæ?'÷ÁJr?"7 Þºé~?îQw":?",flCëª?qRßò«›?nz¤À ?¨¾+Áœ9~?"@Z'`Ü?íîê¶d"?o'1Ÿ×?lÛoÉÜÃh?[€ßp3àÕ?¯C ¥¬–?3x'å«AGN4FGL J0101.7-5455¿Ñ5G×Ò\ÀOÅ?9ѳÀ;»¸¤÷›­À<ùÓ5@"CS/ÒÖ|?öÔxwàâ.?×?=ba(?Ér0‰Š­Ã?õ©óƒðºé?ùÎ
"Ñ¿ïì'œ<Œ?ïûÌ>²mP¿ä#%  ?͗J	
šÈ¿âê¦gv¿±X•~̺AGNbcuMRSS 151-121576?ïØìÒjŠQ?h5k?9À—CN¹?-$¨Áûé¸?qíTñWÉ?g2ØjEá9?ïÈÛ(㬖?y½ù2Kû®?O¦Ù(ýk2?Y'ߊhõõ?wKH
?uöèuù?ï#0ó¬¤R?‹‡R°0¥?jÙ™YA?pç¡Yjv4?˜>ÁŠ8"'?‰;µ½Û{
?îë‰v"d"?'O鏿Ç?gLXãŽâ´?UË<(£*ô?Ÿ¥FˆÕ?Ó2çó?ï·œDCÒ?v§lÁ£f¶?F	Ï:$?:ß!ÜV?€Ú<ó"¢?u·"ú…@?ïe~[ÇôB?"<ëÝÇ?`•jCÃ^Ç?nå°ëF=?'=‡DäRÔ?'i‰2M—ÿ?î½é)ϲ/?''§Ñ¯yo?pŸ'¹óŸ&?wF˜Ü€'?¢
}¦?ç×8bQl?í7°aöÙÕ?Ÿç<…Y€?t²íÔ2Š?qfí:y¥=?´÷Nìîl?Ÿ4"/&—AGN4FGL J0101.8-7543?ì^ˆ!³?CÀD°p~]À:øóºw_³À<drû ï@ú}µ'@'°¤xí?Æ0A¦¾p>¿©cKn?ÞÂ
y?ý$2³=Û¿è,ÊRŸ	¿ä œiàn¿êÙCӔg¿ç"\¾që*¿ïôL¾´ ?ïÀÃþ¬CAGNfsrqPKS 0101-76?ïè3ÄíI3?i•ÀõÐo?Iþ·¡'Ì?Z ¸Ë¥¾?aL¹jeµ?cB$0ĕ‡?ïˆÏÐ7e?‰ßúڄÎå?eZ¾‰ˆju?rÀ†Õ1U?ˆ£œw¦qó?"Ç3ʪ?ïÈÄ2'"?‹âï¬Ò?süŸhߔ/?r¸jøkëò?—§¿¢ëª?Š+^z"š?ﳋèÖî?f»&ÐXu?Vèø^™f
?Eä"ÎÃ?€?æÉù€?dó_ӎ)?ïà%¸¨?j?¿?îc?U
¶âºu?[WW9«§ù?efB'?dœR‡'€(?î×Hæ›!{?¡ç¹ïÒ?rØvô0?'z_×Õä)? 0bµŒ&Z?›Ó~Ä`€?&ûŽÏ?'=;'ÿÜ?y¾¼´3?x¸'$§¡'?¡ÝÚl?ŽH»8Xi¬?îï$ðœ­?‹ˆó+õì?t®¡U.?kÛÿÃ5Ɍ?6H4£Ö?ˆG"žþlßAGN4FGL J0102.0+1639?⎯;}ÀGRv‰ÊÀ;IÍ©kŸÀ<–=u¬T‡@' 'àð@P'Û_6Ç?җýãA?ÊY ãOp?óñIÈ î@ÛR¼ev|?î¥k¼½¿é"c!7ˆ-¿×»d$lÆӿ代yí+è¿ÚÒ¶Ù ¿ðAGNbcuTXS 0059+163?ïÊîx¨Œ?jiìÿ"qu?Nš6ô+?;چœžÃ~?vµ}0xÂ?hin2?ï«>øìÃì?|Mó¤b*"?UqŽ¥W7~?YÝœŠ?''ð|$?x+¼4æÉô?ïI¿±©?Û?™W†M?j†c¸µ^^?h½_Œµ?"‹PŠïÎ(?€"X–®P‹?ï|kÇ{?d㉾	"q?Q€Äj6'Y?5¦8$o¹ê?Ž´õ¦Æäè?dQgÀ"Á?ïzûׯÝ[?'4{ÛV÷?`Ï	)?REKj2âú?:VD®ô?*yZœÊ?ï:¤IÜÿ?òmif«C?^fX?'Z?gâ#"=3·?–Å<tl½?%ôoùÄ?î¸P迋`?VY2^<š?t"Fé´g8?s}³Ž%/Ú?¡èh™þ`œ?uŠÒž¡?î‹kÄ|Ͻ?ƒ¯Ù6¾‰7?`X`öÜ1?Q^ù‹úÑ?¦C½ªQ?ƒ˜–¡ƒÿAGN4FGL J0102.4+4214?ë gã¨À4–™Øƒº4À9°²2í"À<Nõw/@îȎ¤ž@û–¼o‡w?´æ&eŠ@?ÃÒr¾Žpœ@'3cښì@¨§óúc3?ìPSà뾿å¸Â>SwÌ¿êiˆ†a¿èÏ{5U¿ç'kë
¥u¿ï÷§pò±AGNfsrq3FGL J0102.3+4217GB6 J0102+4214?ïùb¥oCb?@(äQ+`?3í2v)µ!?-ÝÙõ{Ù?@~рC"?65+räÊ?ïîd	úß?fe3(Õðæ?0Ux¥~ºP?>Ö«ÔQ©²?_" ì$#?cí-º€H€?ï¥ T˜ê?xÁè:bÄ?fSš{¶¿?kG
Ojž?#q;Çû?sGùÿ'Ì?ïóHîË(?9ÍA±-\?A8¥ç¿'V?(
ñ^iry?PÑÏ7ڐ›?3Ÿ;Q­oy?ïõ–•¶¾¡?G¢Ãõã2ä?Aô׋ª
ÿ?8üíð<?G°Ñ"Ä)?@^4zÐo?ïÇs'{*T?åÞò¹Mn?Ju†oÆY?a¾Ÿ¤~Ü ?x÷»†Qþ?}TbÕM©ö?ï]QkúÇS?†åJ±¤ß?w3"ƒ´2S?zÁ\AÊQ?âÇ5õ?€®ÒÁþoŒ?ïØå £ ?]âÿô®Þ?]Ғ™\?Kїŀ""?h1–ˆg¢?U{Iè&_AGN4FGL J0102.4+0942¿Ê¶¿$·WÀJˆÝ½µØ•À:áüëx‰À<i
fL@ Ά5•8?ûþ·Ë³È?ÒO)~(¤å?Âå+é<ïõ?íúö -G@ãñ@J¿ïêÜ0?ï>ž¡@¿êáz~vR˜¿ºÍ¹†ÉÞ0¿çł Ù©Õ?vCA"jïsAGNbll3FGL J0102.1+09432MASS J01021713+0944098?ïÂêý·?…Ð3^§*Q?=êÐÓ²Ë?W4HÌÂyÙ?|«ÔR|Íz?ƒ°ÜРv?ïÔ¢¯ t³?q¸ˆµ'@ª?Aþ–\¬ò?Jg"˜†Ž?snÕIÂLj?o_jn<Ú`?ïZ+¬Îw?€Xw8¼L1?eNz:œq°?hÀy>œ©2?'»&@¸U?~Ä輿Q?ï>JÅÿ‡?uŸ±Fðˆ?^P\Š¬®*?I^*CŽDj?–ZpäĐ=?t"ÝI«z?ï­9ø°f¡?z¼`˜ð÷?Lt'šj?P™;Üd?'ê@´{ÌB?xôz—÷:?ï}0¥9_ó?‹So÷[W?W£#Ë×u?nDƒˆMPr?¿r=¬€I?‰ò&ga¨?îÚõ—FX)?Š—¤öÓ?nŸŠ}Q¤_?r:ÇÊ8"? f­åÕ'&?Œ™=sëï"?î(¹Ûêˆ0?ŽÚ»8Tú?kzpyYÇ?`ZsË 6?«¼»6ì3?ŽAEo Ì¿AGN4FGL J0102.6-5639¿ÉÕRWeÂ}ÀN3ք³žÀ;¹¯¹–À<¥}xÑ¢õ@ 9†˜*?ÿ›øԒ"ì?ËÞs'êÕ¡?¾Üö êAŽ?îÞx@ƒ}Î@˜ªøè?îÄ8ÿzôé¿ã×ÓÐw¿Þ'•ðŠ¿äþ£%3–¿Ù߈'3™‹¿æ›Ãu56CAGNbcuPKS 0100-568?ïÝ·ÿhÞï?\ÞãN1T?8"¨Öoì¾?(á;šd¥?oC«8mþ¸?[g­ñÙ¸?v­šÇ0?bÊô/:I?S¬ÇƖ
†?Z‰oh»Ô?|IwOe@"?zÆ[᫕À?ïzÃûÌ?t%Ùê}Èê?[ÓÌÉs@?Giº5¹@?ÔÂl2³?scmOý<?ïa·~½?p`Û~=¸?QؾƒÅ9?8¥‰ÉŽE%?'Â6ë¦6?ph¶ê6»æ?ï³úsùø?p\s|Þ}?Mÿ§ks?@^Ð;€¥ ?\b%÷z?næKô¬,?ïeòÖÄ?"yеì^Ù?`X¹a®nY?mºufœ\¼?'Q
Ä­?'P-1¸?ï$à#¬?"!½òÃÇ5?c%Ö»"V?SÁÓˆ?›Ö©%šòŸ?ƒRÄË?îÂ0«]U?t%€gûY?eŸê¦Z|ã?Wel°U?­iÞJ`'ß?×q5AGN4FGL J0102.7-2001?ãòR<ÊÀTœWS£ìÀ;öÚó=À<ë…à1@"m.B]ž?ìHBŽðÉ+?è?àáVÈ?åÁ=¢wä"@¹`ß=è™@f±?R¦@?ìü辚Úâ?ïšÜ?0—x?® Æßwõ/?€3
.ÍÙù?Ɵ­¯Ñƒ¿äè/(âwYAGNbcuPMN J0102-2001?ïÐ
)àµ?k·Ïy¸ó?Qð)!"@È?Fì'ŠÐÛ?szð›7ñ4?iÕÞêj?ïÇÙcð%©?"Œÿ…ÆMä?TeBÔ4?p@PåùK?vùý¤´iy?}½¦¶-.?î孛{"l?'öeSj+?sQYJ‡UO?uø½Â†?žuö@'|5?žg@
?ïA5hÀß?Æ-lü>?4q¦wÙÄm?2…9Ö'Ç?—‡‰"Ž?Á£Ýïü©?'QJî?…ßÙ°:9?hÌK¢\¸?kò}À["?'iÌyÏ$š?lÖt±8?ïxv"|–v?" åȄ.G?`Ž*>.Ç8?wXŠÿü¼?¾Ð"^t³?'zÄg.«?îX&S•˜?—¹éY?pB锚µ…?u`x…`?¨u="»1?–8Ÿ4·bo?î|hLUÕ0?šy_F؇?-
!ÍøIg?:±¾+YØ?¨qøͺ?šr'å<§žAGN4FGL J0102.8+5824?ÔÕ$qpÒóÀ·ê¢ ©XÀ7Ü.u^PîÀ;GŽd²1@@6†@¾‰Þ:³Z?—?úØÍ?°©G¢'@4XÍ!@ÅéôZ/¿¾ÖK¦œŒ¿Þóc9‹<	¿ä->\\!i¿äpˆÿ¢´¿årðR
¿è(ê¿üÚ²AGNfsrq3FGL J0102.8+5825TXS 0059+581?I÷´œ?"¬ŠHTã?UaÕT}'?Yµóή?‹pJ×åf?"Bý1R?ïLÙCõð?§-QßÖÓ?D=h.?cm'Ä\<¡?uªëÀFÆ?¦¢8…Ò?ïeeçTQU?‰Ñ5úÿ3S?q\Uú´Þ?};?ÐNÁ?ø[3W?†"†2ž?ïõñÿaIœ?:\y1É[?dݐÀ=¢?®ôu)#??R•²õ¯EÞ?90ª?îãZêÿŠ1?›îâìáϚ?VÍ䆞0?SÜ2¨ê?¡Jâ"ø€?›H‰ÁTW?íĎ]Xÿ(?·Ý.Od?]Æ%,L²?]yã²Ë¦?±dt€9ß?¶fïgZ8?ï › àÓÈ?''€5ÈÎ?z4USƾ?''Õ$h?•_†ŸØ'=?ý–¾ v?ïèßÌü?VR>ìQÁ?-‰´]ÔX¸?!N$ž»»?eG—•É°'?UŠoîš
óAGN4FGL J0103.1+4954?æ)³»¦+À)ÖV%¦'¶À:o¬)ÜrÀ<
(¼·«Ó@M"àú+@Ä>š4?ÆíG@±K?¶zPÑæ?ìàÛwŠ{@×o?t¿Î£ –x|é¿äœG(³}p¿é½Ê›š$Ú¿æö#l¿êCá9Ñ]¿ïþ{€©Þ‹AGNbcuGB6 J0103+4959?ïšOñý*Z?}¦ñ"¬ó²?d]¯0Ãì?[{èO}uZ?"T—Îg¨m?y›¤•ûŸ?îü­5éØ?Ÿ°þq&â,?gGïVß;?l'è"Ùçj?†ðF9ûB?žw;4"M?ît 4d?"–¹•b}N?ƒô±èLßr?€ä;¦dz?£Á1"¤˜e?'û«Ö‰ÄL?îúújGz?uD-݃]?x"èˆ#T?X©Î$?š›_>gà?rÞV·ò ?îæߊ6½?•vÅâ«cú?yö×·àJ9?nR¹ï§?œ¦XÉäË?"Éà.4Ž?ín
˜U2?·-ó¶ë?€>m
ËuÚ?‹¦¥A?²‡Å›P	?¶CŠ?ìy–$H?¦Ô_QØ?—ÚB†VS›?&I?äò^?¶<¾üniÚ?¢ðRŽÈNF?ìþž
Ç?'I–A¸kž?'e"ᐇ?xñÂ4v^ì?³vxü&?"Ç/¦w(AGN4FGL J0103.5+1526?ywÇÁ°ôÀG«ò<ÈÞÀ:ëCø}T¿À<^1
¿@å´ã¡ûh@ʘÅ^C'?Äé)yËóß?œQö†žY?ÕõèúÕÉ¡?õ­:mº¾¿ïûœÞÈwÓ?ïÍ$Á*'5¿åÞ¿þÞ÷¿ìÄ9ë´¡¿×ãJ<º?¼ŠC:gZAGNbllTXS 0100+151?ïDiôT??'+ÉÙé›?Cù'
ñ?=`¾#²•5?–Þ&°P¼Ç?r6œ£	?ï˜?ò‰Ië?"0­<þ©å?ae	1"‰'?hmi?…–Á?€Ü?§VÐÚ+?îÍ: 1Z¸?"˜Õ'±Î?'ËÏý#ñ¾?"‰Ø'ùÊ%?œòÃöGA?Q1Bd á?ïæBXƒé?yóI}þi?m+´óÁö?[žefME:?™}Á3£?x+D[S?î¼\:¤§Ñ?3"Ãœíú?W@ÚTæ‡?_!0sZ« ?£'R~rº?œs´DЈ?îîsÅÁã?šÑoLR¹Â?pDånKŒ?v‡;ùr.?ž Mçå8?˜–K­é¸?îN.-²7?™‰ö{\Š?Ž#ÏZI6P?Ì¦Ä÷ט?¦')C"òý?"' ·M½+?íz€ÎçG?—f#Ј¦Õ?ŲÝ#?vSBD匈?²àÙ«Ö?–Œ§
ûAGN4FGL J0103.5+5337?ãm!Zå÷
À"gòä¼®À9¼ñÈ.Ø[À<!ƒÞFr@ y:æ/õ;?ú	»…|¬#?µ÷ÝòŽþ5?½³ÃçJý@ƒZ'ó@Þ¿¾qj¿ð?ð?عÚÂ-âf¿Ø("C2¶¿Ü¾ƒžZž‡¿Ú(ÔɎÕAGNbll3FGL J0103.4+5336RX J0103.3+5337?ï×J¯Ú+?n`4à×Z?9CôFü*?2ÄQïî—ä?rç›d‡Úy?mpF	´¿§?ï‡r,9¼1?"¬¤ÙÖ°?DYñât?QßY‰Wo?ŒÝÕâîó?"³Æw^?îÉü)u‰?'ò¸Î–?s"kx¬_?}•]3‡¢é? íº?Aäp?'¡Í»LVL?ï^#d=;?rBlé7¾•?\iž¦]7?DZ:Ušà?'tùœÑ–è?qLÜ^[œ0?ï·¨ )z?{‹åÎ3N?NT¥nf>¶?F£ýŸ×á?€0 –ÕÆ?zfè¡O€?îÉÎÉ.æ%?®‰ËÃÌï?TÂb§öAÑ?jßóôªy?¢½TxM%?®JvׅŠ?î£e}æ¾?›•¤ï??xëbê$g?pߦm6j?¬X]L&î-?š2µ¸GÕc?îÍњ
Ä?†Ð½ÏP$?g÷,á!P?[Å»Ï7)õ?¡£s|¿?†cj†Ò.ÆAGN4FGL J0103.8+1321¿ÕîÄz)"ÀH³ïàÎ'À: ù™´qŒÀ<‡ú'+6@ùOH<¯´?þê»m(ø?ËBq¿ŠïÞ?»šÚ¡Ì˜õ?ðÖáù"»¼@³!€nÅ¿Ù"K"bа¿ÓŒIåQS¿à*;½ÆI¦¿ØrÁžEzÞ¿åSUèiáE¿âæqqAGNbll3FGL J0103.7+1323NVSS J010345+132346?ïøÄý <?6ŠE·û§Y?xO'v/f>ý¯²wKAÎ?JÜÿéSâ`?5Šúp3×H?ïçÏnVŽœ?i%xá?.ƒ+²Œ¤?>«
c'íÊ?fH^ÀŒ?fˆªŸ­…6?ï¼ßñ[':?iöÏ÷Aôü?Pç±C@?[Üy	K™4?}VðB‡?dÚqˆ%ü[?ïÚV†r‡?JTïŒ?"?1òòtÕ×?œðùõE¦?qÃ<£ôå8?IŠÄi+½{?ïòê­!O ?F"óüU‰?(Ü;ð?f†°íÊ?XicL|Ě?E¹è²UÁ§?ï¸Ñ}êA?€ç²¾È?>âcÁ¢n?M´Z¿nÜ?€Û!rD)?ô]@•õ?ï–9–Š×›?tIqGÚ¤?Si ¬Ú%g?C¹1ôs¡º?ˆfT
l|?s•ð'ÕÚW?^š¯?gìãYµ_¿?@?ùâÝË?+¥sÆô?†4Z|W§L?g£YhyAGN4FGL J0104.8-2416?秮%¨í0ÀUv<òϕÕÀ9î
^u×À<|ŒbyqÜ@HÇ nM@>Vð†?·‰áÚiÝ?º!²¾iîÂ?ûúÊ8Ö@ Î|O[Þ?æÇ¢u‹G¿ã¬ ‡t~¿èÉ—ïun¿é£J‡ãŽ°¿äæZb!2U¿ïÿÕ7ÕYcAGNfsrq3FGL J0105.1-2415PKS 0102-245?ïòÒoùã?ûïÓv¯ì?f6ëêܵ?õ8/í5]?X"¼Téî?ø܈<Î?ïÛ*Î_Éê?€§íó¢Ÿ^?33íêDÜÐ?Dì‡/Äþ|?q7YáÝP	?øz€TÑ?ï©
—L|?€M.ÄÔÿÎ?TK>RX4ó?U6HÛøÏ?ƒ3òsl·?€WõZ?ï÷Z¼'ýº?2Á,DIÅ?+$hDUþ?BbÞ®ê3?KÔe«D?0åoké[Ø?ïó"a,{ð?Q‡N×=ý?*,eM,Ó?"‰?ÓV^?U"±w…I?P»J©±C?ï´ôwqâ­?Xåf¥>?Eô͸Îj?]¬Õ©Ê?c•;g~?Í`Hÿž?ï_ÏïÓ?‰Øù¾¸Ü?`q''´æ?a'¿¥…×¹?'÷Ñk¶?‰¤ßÔÐø?ïèäz	ÿ?SÆ9\°k«?CXÛôDÙ(?5¥Z—:‡?cä€þL?QçqSØWAGN4FGL J0105.1+3929?!t€À7Lq²•êÀ9åق½µÀ<m›2öÍ@ó	WA°O@ß^Ö?¶2«M÷?´ëÿ—û3è?üÅ,ÅZé@‹&NÉ;É?éRøàÑçi¿æÈ8–¿ã:âŠú¿âŒ™ÖÖ;¿ìæÍߜ]C¿ÜC!þ,–6AGNbll3FGL J0105.3+3928GB6 J0105+3928?ïðc¨¤'	?P@Kâ'}?2ê8êîÿ?'ú-–Ÿ+R?Z~!/…í«?Lܶ¿x½?ïìÚW`a?g_Å &'?1D-"¹ê¥?@©&‡F?`ý"÷B?d®îÁz¯?¡HJÙ?'LíUmÅ?s"§9Ðf?|¾óåÒA«?}''Ôí?tÈ·œ•s®?ïîâhž?@(v†ZGû?B*+'QÆå?&šÆ7ìkå?ZÃ% ú¿*?;x…Í
?ïäd1ò…2?^}çÂæg?Dš¦K‡J?:bUfåw?fk',ÊýU?ZeúhôO?ïÁÁÞÝ£?'úGÛ¬Ô?H""FØ/?\½/4›Ê?|¿þ
ð?€øL"l¹?ïsHG8ñ?†ÂŸ#%±Ü?y	Rë."—?ê½¢ß$Ö?†"!»j?zY™ï¹?ïҁÈþ;?^Zñ1ÞU?W/¶_?Dþ(§ó«?póX"Rîæ?X""óõÿAGN4FGL J0106.9-4832?éà:ÓÄwÀQsWæpãÀ;råx+‹À<îã>ÿP@+Ç¸æ¼@±¦»ÁÎ?ÉW_ã?ó¿³ÍØ®?ã,Àþ7~@¼È}‡À(¿ë­AJÅ¿èpúß.Ï ¿Úò yI¿àIÏâ€é¿ïÿ¶.$Öy?ïü¯ž=Ã/AGNbcuPMN J0106-4831?ïÚ)%ÆÂ?hÎT£þœÞ?[M#2­ÑÞ?Tðª÷¶ÂŒ?hHE>"¥q?bŸ'ÑiåX?ïч`uÐV?wûV@}m?GÍ´—–MÖ?SíԙFÐÛ?tB™GÜ,ý?t.û,éèp?î·»óXG?"ÇçSÄtÐ?‡"§KYN?ˆ§;۲ʖ?F-ò覃?¸Œè Ö?ïãàl3Q^?SH°³ß?;?»íäIË?* QӜ°C?h·œcùN¶?R;х©?ï¹µÛï?uÞ
!ïük?nT¾9áI?h
@–ÜB'?sú³,S®?mmí¼W÷?ï7¬I
?ŽÝVþV—?WÌØÈÇò*?d~ìQœß°?Œ¸Ÿþ"nW?Œxö7´Š?îG@"Ãì©?˜ÃZÎäœ?…Èìš&ð?ˆb…nÇç?¦»7yb?•ª‰í.`?¢åó?uçÇKAë‡?T	NÁ¯¼^?PC6÷šÖå?†Sme^(ª?u®0*CcAGN4FGL J0107.3-1210?ëM2éqÎÀR¦JŒL˜À:ºœiànÀ<ŽO'…€@ãg_ƒH@8>ž¡?ß­¯Ñƒ?¶ÊÿB?ë}?ó>~:˜'B@F
ú"†4?×·IbŸ‡o¿ß@zC'ý¿ç*
Osۚ¿á}¸èi¿ëÆÏ\Ê¿º¥@v'AGNbcu3FGL J0107.0-1208PMN J0107-1211?ïÔï['å?c¸ä0æ?IwµÒôŽ?:íPÏî8ÿ?rY[­z?a¿uú?»?ïÕ6äÏð?r>õ‰Þ~d?CéIòa%2?K"
b¯?rçÉí½9ß?oô¿•æ¶u?ïªR±Ó¢)?rŒUÓb
?a9ú«Ë?iÝn20â?•'N¸?j#.–0ý{?ïÃö.<uÉ?T—p °Ä?Q¼¹–Ò{?2uNåh¦?y•áñO¢¥?SxÃÁyr3?ï'*Ÿø?v .4Ïø?^Á-Yñã.?Q\Ù{.S?"ÞÊq» ?t î²,¼ç?ï']ÌӜ?ˆN¦šø®?Tഘû?b™»žÃL`?ˆÌvE ë?†TÚpûõí?ïoPSe¾Ý?*êÛñª?kµ¹W?tRË}7%k?>ªarH¸?x®dŠΌ?ïPÄØ.!?u2Ž¬ú?h19ãðb¦?R5¸ƒÊ'g?'ù@' Hƒ?t‹}ëžå*AGN4FGL J0107.4+0334?Ô<Ôÿm«LÀM‡æÕw–À:ˇõ,ggÀ<_"žy_@½$x°?ù@chºÔ|Ä?Äs¨è茿¬/ñ¤|O?â³Jå×_Î@Rú_W(†?ï–ÄÓG³¿â^•ýWÚ¿äæAGÈìm¿äpý÷<7¿Ös©Ïr¿ïÿò> wAGNbllPMN J0107+0333?ïéóöK:*?f AÍUŒè?5	ŸnØ.?0"t"H¨Ë?cjՔz(™?e	5öixÉ?ïæß	æ2Ï?g¼OW¨FÔ?/Åw"L§°?8ÀŠS¥?g$ž½<Xm?f*s,°«?ïšò'œ…?zQHßMF?X°ÖþÓ$î?d¤hÇkU?†-Dz¼k?x+•Ió§ú?ïܼ»Ôú:?Qr'¶÷Þ?''©|KÃë?§»v)P?påÉæã)?QT*§ó?ïÜóòß?o¶u=àÞl?A¥ê=Ä÷§?5	1ÿI³?oŽ'ªÄ-§?n§öGP;Ï?ï»'̀TW?ƒ;Ä|5?ByÂ`pÑò?Sþ–-nD?€p½²\?ðäA{%?ïIwëtÚ?†LÈ\Zö?`¾ÝPs¥?ejz(¯[?"¹&âë?…) €k.Ô?ï‹aíª?rŽ_h9l?BŽig¯€?6…ŠÒE'Ü?‹þ»P[^·?ruÜWY°,AGN4FGL J0108.1-0039?î՝þz'8ÀO_ïIÏÀ:;+@ªÀÀ<}7%@'/m@§'…€Þ?Ä °¤£
?·p²o©[.?ñƒSV¿)v@Ph$»¿àd¤à¹)¿å[ÃÀ^ªZ¿è{.¿±q¿å¥ŠžT~¿ïÿªoª²Ç?¢''%ߍšAGNfsrq3FGL J0108.5-0035PKS 0105-008?ïàˆksìa?bW¿nê=Q?Oèñª¾ñ?F½îu¹Qb?g}WáÏ?^3>@	‰Ü?ﬢ'‡®`?s·z²¦?]#0O¶É?d¸9¡4p?'Q±ƒ/G?|*¡›É>?﵍k
?‡ØżRÐ3?yæN7»:?wÇÊcvÖü?•ÏºÔ,¥?ƒ	í'ØÍê?ï`6M2Ò?q>]/ÉWá?o1¹"cf?S¡ý^ñ˜*?ÿ-"…*?oƒéË?ï²@|që€?w¬á€©)Ð?cð`Ó¼ïw?]Øø˜JD?|ç'N½lx?s•×|-¾?ï
÷÷Œò?Ÿ¼x͹_F?rCxQŽ&?|bÊNê.?™°Iª1?›ÅÛϛŸˆ?îüÊ@€y?™ Šs'È?ŠYO9"šX?ƒ¢©	p?¨Iߎn¸Ý?•C^êë?îMŒáám?'
}"
È ?‰rèz´Cl?v°HYKzò?§þm€[L?ÜˌI¾ªAGN4FGL J0108.6+0134?ïÔl+!kàÀN~ß?–À6ÉÁö¯õ&À;)׆d2¯@ìPGk#@FtÃ÷;5?†j½ýÀÏW?º²ËCàª@-ùmL3µ9@!‰q S²…¿ËÅaž€‰¿áÆ,¿Ñ'®¿åû"y™¿æPÕÛiH¿êk¹AT´¿î¤;I'*AGNfsrq3FGL J0108.7+01344C +01.02?ï•h©PŠ¡?€|rýXœØ?bî'Æð?`+˜×Ì3?…ê4ÿ '?}ŒXç@w?ï®ðeO²?­±4vòS.?}˜ˆ	"ÍY?"RT?•ãÿò¨¤[?¥¤ý±Zž?îe§F!ï¶?¡ðÖVä=W?¢"2or?žä‡¸øWá?ŒId«ƒÚs?ƒÈuDè¢?ïÅÆWV—Ö?v'".Ú-:?dùW£4·ê?fE"Œß€?r (¢¶ ×?k€oýPê?ï˜ã±ô6ý?€Jˆ1¹õ?bˆ5ïR?1?aâ4Uƒ¨^?…%\Á?}
_â	?íȜ¾?º×Râ¥üÿ?"Qf'Æà?¦ÅïŸöÛ?©Í€Úc–Ü?³Z:qŸÔ?î¿dÒ[?œ/}'¾=o?™ ÅF!¡?–=<åçå?þuÞ]×?—Wô(sv?ïUDAÅ¿Š?æ»Î\JØ?yXë«î†Š?x¸Ï)(ó?Žy²˜U?‰:ýƒ®2ÉAGN4FGL J0109.1+1815¿ïý"#–]ÀF3¬ÿiÀ9'Úa
À<8.j€@q©(ؼ@cH¿Œrj?²µ÷‹'?¯Èî_³]ª?û'{Gžû@?Ï y¿ÜÜCB	[¿á®†ü#»¿ÜÎÊ}è
E¿áäÃßt¢¿á>yî§z¿ìþ3!?•ÂAGNbll3FGL J0109.1+1816MG1 J010908+1816?ï{è"‹¹?…ÞM몺R?`ù¡ÚÄPä?X¹YêE}?ŒÇŽÖdS¦?ƒ—¹K6ôW?ïDp•ƒ#?«\ñ—ŽOÚ?oFU	&ÜA?€Ç˜ºuì?"•§KÒÊ?§¸J;(?íê*ÞÈD?žM6¼¿?…ÞÉ™KV?‡Í?ß'?«ç뽌ë?œ›eTêÿ?îÏŸÌã?€¼iA%þÜ?€2t¸0?b†&$uãÙ?¢'%ô+B?}¨t™S$?î"ËÕ+?ž¬Ûߝ ?|³1;¨tî?w(¤rfS	?£8½Ù‹?›XjKäŠ"?î3VâþK?°m'.š?'ÆЧTo§?—Y+.EÒa?¨Ý´‹m?©îЇ†5?ì™V\qß°?¥×.nA?Œ²œݓó?ˆœDm
¼?·žù—ëuƒ?¤"'‡?ìÀJÑh¤?šk…¶Ã?'ú‡bbàE?|ó¿#¼r?µ?œ"fM?—ïlΤ,AGN4FGL J0109.3+2401¿é©ZõÍ®ÀCUGNΚÀ;¼|óp¦À<xwiÃèø@X.8¢ˆÖ@ç¹Å‰­?Ǭ0,–¿Ÿ"|Ái
Ø?ÕZ@ÿÚÁ@‹›˜w?Û¯ç#e4ã?ãeC»¿ê$kºc=½¿Ê[ê·nkÿâ["ötf¿ïÃ;ã?ÖAGNbcuGB6 J0109+2400?ï×Vå®´Î?j}‹¬&%7?2êÜÓc=Š?(Ì6'´\Q?s%ßlE{E?i³À«'Ñ?ïÕ¬vYèC?pßæ7•‹?9Wæýdï?Dÿ¯èƒi.?s"Ræ_x"?n@a~|*?ï~Üc¤N?Í'~O3Â?\¸g‰ܶ?fѸåÔK—?Œ±ÚMÖÜø?€û¦}ýa¸?ï¶ûïq‰Ò?bIxN¿€?DìÛV³?.<Sû;£Ê?€ò6j'—›?aÙ ¢NØV?ï«p¦R±ö?x‡–õ•è?EW'>xÝ??9íÑ\aÞ'?ƒÎ]:¬šñ?w?xuc'§?ïŽûk¤Fy?‡#…Õ½B]?HÙ=´?VhîzuS?Š³"ôA¦?†Ó]çe?ï>µSà?Ž	E/&a¨?bŒœƒ"à?gv®ãÐÅæ?šæ¥Ð"s_?Œ²'2oŸè?駱‡ ?¶ýóU`¦?`¼*»Yü?Od—ûö-?šU?ö°¹?hÈ
›ÚAGN4FGL J0109.7+6133?ëJwçݟ¿ó¸SH|p"À8-Ðé'ÿqÀ;áÝÖ	Œ@"ÑéÂ&@""ãw3=?¥,È
`)?Ä=2»i"-@–6mzVÞ@hZm߬x¿ºÅM~¸î¿áœ§ê9¿ç΀2ÀG¿éokþUÛÕ¿í²˝!ä¿ïÿŲýîAGNfsrq3FGL J0109.8+6132TXS 0106+612?ï8á.>èÚ?°°~_"ßs?'»'|»u3?£'ß:¶?1ýÙ(3?°û~&>?îR/&è?·,Ɵ-¤ ?T¨ýÿc'º?gV)¡öÊ¡?ª2§î[ö?¶ï4óÖ¼?í"O¨BC?£ÅWþ誃?¦¡Œù•[0?ÑJ°´Z"? Çšý«?•åš@½È?ï·T¤do?f˜k´•†­?Y%¦çŽ?HÌè¸õS?~J,q<¡?c³ã çJ?îų—¶Y]?›2ªùȖM?"tLJ^݁?"-‰ea1?'Õ@¶>ðö?‹¸W!ä|?ì¥Ç>1X?Ějö3ù?r¡\¢®)?ë?S§òÎ?¾p¼bÛ?Ä_³ÓÆTý?ìÉkƒÜ˜ó?¨>>w[—†?¯SšYMC?£Íã…ó_ä?¤­k|ˆŽ?™~O˜?ïó==¼é?ˆÅõêæ.?véM+øS?jôà—ýÞ£?—'E3Ò?…ÍBBŒAGN4FGL J0110.0-4019?×5÷UXïÀS™Ì¢ÛÀ:õ"£Ö3À<­9©nù³@ ›èÔ?]?û!³Éƈ?Æ	E£ù?ÀüÆ$<k?ú÷YhQ"@¹ˆºa¿ïÿ¬=`2Æ?ïí«3õÐÒ¿Àµm ‹]¿ÜϞƒŽ?s¿èU²Ÿ$?ÑÝсèMAGNbll3FGL J0109.9-4020RBS 0158?ïóâT7S˜?HU	¬Ý\?(ykÒ«‰L?#'¨]–Ÿ]?U,*KÊ+!?E¢¡â§£?ïåõxp1Ê?mÙÕ÷7}?3uj\·ˆd?@Bÿ4?g›ÚI¶¥?k	L]
e±?ï ÂàºÀ[?y²çùÄìŸ?U"´G1MC?\b3ˆ?…*ñO íš?xH¯ú_©G?ï±ä˜è¼?awü½Š¢v?K³!|:ÜÊ?3ËGÿcR?Ë§°øù®?`ËØZ€"?ïâÞÑ v?`†#[Öë·?EÆl³^Í?Ba°àbJ?g¯"ë'«i?\‹Q@³#+?ï¡âÜaG÷?‰e¨#Ÿ?QY›ëâ?a^ˆâ_x?…\d2†?†ä±Z€?ïb
5jŽ?"®ùv§¾?_©´Z?Z—?fi©¨Œ¦ï?'þ^¹Ÿ?'æ—_h×k?ïK¢¡'Eô?z–$:Ž¡?V¿€Îâž?H"{Ð9'?•»ŒQ•F?zRY»F‹AGN4FGL J0110.1+6805?áàÀ­Ù©@(X¡ÅgÀ8qö_mMáÀ;¥Ý·Ö›ƒ@ %jvÁRp?ÿʘû(¸?¢6ÿ#>Ò?¶n]øû÷?à¡s†Ž$@qÓ%V{¸?ïßÑ÷®ø¦¿ßA–bØg`¿âýÝÄ쯿ݤÙÿj+¿Þ…"/_i¿ÞJ™¡|<AGNbll3FGL J0110.2+68064C +67.04?êïß#?´H¿†Ý2?sRõË´±?eÿY
ŒÄ?Ã¥ëèØo?³ýBâ,úB?뚨űzŒ?ºü›Çq?}lñØ»g?†›1¼i?À­Q€êåÖ?¹œ|‰#»Ø?댘€…?ª!"² ›x?ÑövL4!?Œ£±Z"õ?¿¥$oԁÖ?¨eòí%?í Ù&ÕàO?'Ò£vHMû?–:ÁßîC"?zÈclÈŒ?ªÕ¦u;?‹¼oìÒË?å¯@þÖ?¾'ï،?†âfÊÐ?z½W& ?ÓêÀŠ–"Í?¾s‡Ùu?岊ðù?ÊBFݛ7?ˆŸî
|?›£àük?Õêv«Ù?ÉòA'´ò2?çÓn<§-ß?²>,êdzb?"™ôåÞ?‰6¹É'ŽE?Î?qœ-%?±ØÔĝ;U?êÃMHCvÞ?©FÅë¡?ª¯s©"¬?•5ód¸§¬?¼ž¾5y4?£o9AÓAGN4FGL J0110.2+4151?àöôAl<À4à@žUÀýÀ;¦ºq€uÜÀ<Ðà`'ˆ@"±ñ°Ü×1?úH­ž3\N?˚R¼iš?'òk—Ó›É?ʉ8x[@¦èxyä¿ïÈ8}õÏ%?ès5Â¿æi
_¹ùá¿ÅJâ&{>æ¿Ï&ż9¿Ò;lˆÌÃAGNbll6C B010709.9+413321?ïá¿îBt?a̦>÷R?$¹3P§?NÈ4¶Eì?lþ8É*ñè?aX±ˆà?ïÙ÷…]!™?u¨j'þô_?8ÏS~Ši}?Gù9Aš±±?qwH4ñÕ?t'é'ìˆ?ïIŒwª?"à™†B?VîBûc?a[EU´W?•l߈X'?ƒˆÉˆaÈN?ï¹®ø·?i›îqÛå?7–li?%çE"è%ý?€ÿDžÄf?i¤¦´¨r^?ï¾ûnSxV?q…H«?3"8²?'úÄé€Ø?IX)¢g?qAëäÌä?ï…26Þä?œ‰–‹*?KÉj¸"T?_¸&Ørü"?ŒþœÅÌg?šÕV·"­?îÌߧÎn@?<H34/¾?W®\U]®?[u"ìàO?¢y ~£?üÀ?ïZöƛZ?ˆì4cbdŸ?N¢TÆæ¢?Eûn͕¦9?œÿŽ¯ï?‰֗VgAGN4FGL J0110.7-1254¿ï—~à–êNÀRÄéÌ·ÔÀ:¾šþ§±À<Š®ª¢ÖY@½iLʳî@Pys‡?¼p1v´½¿–û^c@J?ÞÔâÛVþ?@9ä>-,?ïÿQ÷GË?ãÙª*áU¿æp·'¨å¿ê\Ïä¯B?µ¦ï|¥¿´Af|¶´ÝAGNbll3FGL J0110.9-12541RXS J011050.0-125455?î=0­Ðeç?ÂË –§»Š?Gpˆ'+D?CUïf<QÞ?«Ï4ó1"}?Âεð'NÍ?ïÀRbùI'?…ÝZÓð‰?Px0€_èœ?Y˨ӧì?{¸Âz œy?ƒ"x8`›?î^—@Š?˜Íe(AËN?r©»G'?vDÿ÷7'¶?§¾6½‰@?—ߟÄG?ïtG¤ü›"?t:W' Û¹?O*L†‡Oó?A)Ô»þQ?}¸ýO?sæJr  4?õi?¥ÞF¢š/?Wöø㊸-?RàbreI?¥÷Vêñ›¦?¥È£`ƒ?ïkåzSêI?"Jž¡Ð¦Ÿ?_f
×l?rPwJ4¨?Œïët}Œ?'œËØO?ízW|"¤b? Û6
í´?z¨½ðÜ6¥?}‹ô"¥¿?²'¸=Fþ?ž'ÅNyÞ?î9gf…^é?"ôÐÐQ6Š?h÷ÀI;?cǁürk}?ªÝN!¼Œe?""Ê!Ì®oAGN4FGL J0110.9+4344?ᵊ<À2ûÕýÍö˜À:Þc'í"ÓÀ<Šj}L[ù@"'ÌñŠÇ@á߃ˆ¶?Á1¨r¥d?vëþà(è?½ªñ°±ä@Uuów0Ž¿'…ÅYïh6?ת#Õr8¿éâ6Ó¿é ž9$å?Å~{
ã3¿èŠ= ÿ:AGNbcuGB6 J0110+4345?ïŸô5?˜XNâq?^
ãïYcÑ?y'¼ò4sy?"}ÃJ4X?–,»cf?ïäJEði?o4Äª?1*14šÉ?<íH9Ìø?i¡Õ%¬z?m'ÓÃÀ@n?îìø¯'?–ßüTyÕ?`º4*¿?a•rs=!? *èÓ;òb?•ãîz½"š?ïè_k4?KkÉþb¨ƒ?%ÖÌ5]ó?S™‰DÊ?fˆ3د
?J¹ô¾î?ï"Ï0|Ì?…
þý=ÜC?[^šM"–?Y÷<©%î?‡``¢^›?ƒœ=\ZµŠ?ï´4ÏY]Ù?†Ù‰žþ?B¼u^`d?UzuRÎ?ÇJ—"À?…°í¸@E?îýÙàº? uÒ
?g£ñ¡'?jR–'.?¬•ãTK¹? ¹Z)AB?ï´lÓµ@¶?ióñ^éx·?A…²ËÅ#'?>ÖAt}Û?Ìoò¹²?i®ãë:ã¹AGN4FGL J0111.4+0534?ïºB_岑ÀLxYÈÉ2À;r.´ƒ*À<À±Ù+€@ Øp±?ýñ´âg?Òص8[' ?Á8CyT?í6ͼ¶Õ@p]i!­¿îù/Lñ ?ïý°šgó¿èÆvÁþ<±?±e'«é¨P¿é.&ïX¿Ìò¦%C1AGNbll3FGL J0111.5+05351RXS J011130.5+053612?ïóŸvŽŽ?JNh€ÛŸ~?*ŽSAÔâI?"ì¢pNçÛ?U'öéá£?HšœdT\?ï蜊uöc?i—	»Mp?0ìZ\qé?@Ó¹dÙ?eEêuu<3?góƒO•;?ïv=ÛÎ?~ŵZ+ ë?`<JW=ÞÆ?go8è>ñ??Žav¡ù¸´?|ía5-Ã
?ïÀ°ÍpiR?`ýD‡ñø?JÐùüU?76qH?|M—U!:§?`p}"Ž?ïç¾D§ò?]ËÛmFýÝ?A¸Pê"ï·?A8dzÎ)Ò?cÓ׸£?Yˆ œ_¡?ï±Úéè^?"Ÿ'˜?DÂ[öì>N?VlØȼój?'mc}\ß?ƒ7mŸ&¶¢?ïĹ5žÑ?ˆ3úA?eº/ÍÀð?kõ­úKKˆ?šÐïŠÛÉ?‡#Ö°?ïa÷÷rè«?{ú<ÛÌC¹?Z¨R9²?Q5û6-Ò?'&‰Âç?{‡¦WÐüAGN4FGL J0111.5-2546¿ë­Û`ÀUR¾7ޓŸÀ;0÷b¢Œ‡À<¶53¾sn@C¤Ýšzj@'Ýãu†?ڊVwÜ?È žE¥Ñ‹?íÓõƒ¥@	Óf'Ò,¿í!*¢jùs¿àÈ3?Èlì¿ä^1¾éà.¿áp—AЄè¿ïü楻æË¿ïdÑ`…PâAGNbcuNVSS J011130-254531?ïÜ®Ò:õÊ?¢–iþë:É?dzÌÂu?™£o‰ºNQ?^ue®—Ää?‡/Ùé>=@?ï۔c#æº?rÞ!"½E?>§iD?H§ÎÀ¢/?pKWßy{?p©úmÏ{P?ïYP¡œâ?ŽI2&'p"?n,Süô‹A?v—Ôý?'kf*^?‹í\ŠO?ïÑßÂâ'?UÁ©{Œ"Ý?2Ôî.Uz?§]kæ–Ì?uâϛ›ÀÓ?UÃÄU;?ïÝ^Ág¥?pæò)d?UÛýK­˜ù?k5Û7€k<?g³?Çèú¼?a2;ù2?'áqþ? ÎûÐB?WaªÛ±z5?g¢diš!!?‡¯æ,Ý=9?‹Xøºrtj?ïٝŠ¯?"éE"¡?s¬Cv¡?wTæ@¶?šÀrY5fÄ?'Í2"g"?ïŽ-ú(‰?vB*çÉ5?9¥‰|…mö?4ÈSŸD{?‹§U#Zé?vG´$Ú]AGN4FGL J0112.0-6634¿Óƒ·*à9¢ÀI6<tûT À:S@FA,ñÀ<•Ór²@ߟ²ãA®@gFÂú?¼˜ðý-½¨?¾
iõçù#?ýŸ¼ÉIŠŽ@	š"‡0áI?ϓ˜8E–¸¿è÷̊‡­ß¿æf'Ï ¼¤¿ìj`%څ¿åÁ/ÀbY¿ïöm_~ë˜AGNfsrqPKS 0110-668?ïù¹Ùc6?=dRã©®?![F84g¶?AG9Äb¾?DÁË&#·U?:@MA	1B?ï®ÍÅ	"Ø?†ëŠ«~Ä7?X©Abܛ?oÚÙ{l?7fœ2Ð^?ƒà({?ï ²
1dÚ?
úŽ®Þj?UˆBi¿ß?U"M¿¥k»?…"u6=Ï?}LÐ|%ˆ¯?ïӆŽ5H?Rðø£æ]?Z
Œ0‡¹?A§,™Å?ot+õËúb?Nâ׋oë?ïè³T¡?_D"·a—?<C¿l?6 '§"—¯?cÄIÿTœ?\™J[ô=™?ïÂÎ`¢?¡£FÂaWì?hðم?vH0Cb'?šº? H"hìšÌ?ïRæ)È®ä?‡ZùH?`A±£&Œ?`Ë`6¶è?"›—ƒ-¶?†+U‰Ãdy?ïoq@ÎÁ?wàN$ÌKF?vŒvLÖ?e>Ý ®…•?‰éàG ?sGðÄu¨µAGN4FGL J0112.1+2245¿î$¡
¸PûÀCïmÁ¤zžÀ7MØYÈÉ2À;%IfË@'P¹+@¼Ú'.?'/,¾O¢?­:­a2Ü@.&,ƒí@2od;黿"ZUû£é˜¿ÝŸâˆö´'¿á›žV—¼J¿á1xþ™x¿ãò«G£¿çåøL­W¼AGNBLL3FGL J0112.1+2245S2 0109+22?ïÜÞÝgñù?…Íj;C?B¹¦ÂÖ°È?Z)fš*›…?nr¸éôÛt?' þ»¥é¤?ï·¿a Τ?…X'n¤"z?P£æOûr?Zw.GU?÷UõEŠû?"­–çè¦?ï†v¸ÝÆ^?Œ…ÉèrÃã?|¶\ñ:(?†íM=#?€#_&"T?''šWç>?ﱛ¸,"?iÍõØu?Måå]Îx…?;·Ænãó?ºà·HÃ?hG¾->Pï?ïÓe¿ï¼?h,¿l*?<½L^מc?7J¿¿‡ÝÚ?tK&ìiO?fõAÇ0ç»?ï>®
fg`?Ä«7ž[?eÏ/£¿¶Ü?w>Lh!Ë,?•pXenZ+?›Hø?·èô?ï"yÚÀ!?ŽDô2àK?z>dÚ¨?…RN€ur?àjÅÎo?…0ïꑷV?ïd¯²q?!ñòÝ>?[(%Ù?N"ÊèÎj?'·œÎ}2"?}öñ±Ü"*AGN4FGL J0112.1-0321¿ìK¤2œ+èÀPnk΅3±À:MÞÌ©'^À<YÙAOU©@sLYŸÙz@Öðd‰Ø?ÁË©â,£?ÂÞt"ýS?ýJð
­@IV‹'?훀#¦Î6¿æþ*¿æèɂ•q¿ê¯ ²¿â¦=Kºéu¿ïÿT©¥€XAGNfsrqTXS 0110-037?ïãÝ?`¾?\ø@¾k?GçøPeaâ?=ß8ºÊϑ?f(€"oP?XwE‹—NÄ?ï³M…Þ?lq$Õ×H?Z©'u´,?c$aMÁ?®ïNOkë?|: ç‹"?ïœ~nxŒ6?vr•ª5M?]coׁf?XÀBdy]V?…3ö]²H?txÏÈsW?|@dÁ?fS$ÅR|?a˔lùÈl?GS[pît?‰ßûÑ譍?d–_õSi¸?ï¢Î¡Ž/®?}G×%/€?a«>Sñ?YºSÅoKj?'áˆQ…x?y•Æ~¾œ¿?ïB#ƒÊÐ?–&zøu›X?mÌ·Lç?{ó3[$¨|?"hÅ~^?'"óŽO?ï--‹ºš?‹i&)ø[x?kÔ»ŽúïÌ?b氇˜€?–ß·pÚð?ˆÍ–"
Ê?µ$Ö?ˆ¯~L%?zÒÊ­'Ë?g9ˆu?¤,+Uc÷±?†
)¢ÜPˆAGN4FGL J0112.6-3158¿ïÂõù@ôÀTÓü;OagÀ;®¬A<
rÀ<õË^7ü@ m®@o±¿?ö
þ`Ï?ß]àÛÍq?ç\3rSÎ@"ìck	c@ÃüÏHýö?ê³rôb³¿ïÝHæ"ß(?ìM¤=Œ}|?¹–@bŠ~¿áÒ¨ëÎE¿ïùêqùA AGNbllRX J011232.8-320140?ï´E¶‡Tâ?•ëe¬;º?`×lþÿM?•—úX±?}q¢æ9§a?Œ…;˜ÑUo?ïP¤P_qˆ?¬sóýõ+?qqÔ8½êé?ˆr_48?'➳C?§ÞPn1ªÖ?î²`ÃlÚQ?"ø'}á;Ì?}1Ѷ¤íå?€Åzü~ñ?¡3¹•o¨?"fg˽Ä?î 0y;øv?Œ'rEþÎ
?Zlæ
?L|wý—
?¥)'>™RS?‹ÿ8Yã¡%?ïƒÍদü?Œ²J—2I?oòpï°^?i͗Ù>4ð?‡뢩Le?‰õ²ËÏØ?îâb-Fµ?°zb&¸t?y]øó`#E?'ÕuÌÜ?\<ÐÏ?«]³|~1²?íɑ]ØDÇ? LŽ¯ó?'T|m®o?"ú%˜Š¼?®ÑË
ìg?žËEŸáÓ?ìÒˆóÆ?§ÒFt³¥?c‡¸ðpƵ?eDkCÐ#?¸Ó%ó?äX?§òÇâq¬AGN4FGL J0112.8-7506?ëûäû RyÀDù}¿HÌÀ:ZíÍÎTŒÀ<'йÁWN@»Þû£yí?üž_ ÷Ç?ÅöX¡×«£?Ëë4Áӟz@@ìYZi@Þ+"ƒZ=¿Ñðh}—ÛS¿ä¡ŸAÏ-O¿à¯¤Ùš¿Ø5X§ay¿áá»;ªÐú¿ïè ÓI¾AGNbll3FGL J0112.9-75062MASS J01123146-7506179?ï˳'M¬?gê0V¨6ú?S֞_4™"?E«+j¶m?u}þ˜¬Ë¯?dÁP&²ì?ïmª}y?ŒTá/ñ?kËœ)x–?qtø4
?²\MÁ{?†.­ÄG7å?ï"Šar
?Š#Êö¸øg?€<ŒJ–9?€‡÷ ×ñ¯?"m³Ó$×?ƒ{ñðÍ"?î–_ˆ%ÓÏ?}´K9ï|?ƒÇߟêl?dŒ-àz?¡¨'‡ q?zšó&vãì?ï'eÎÄ|O?}¨Ì´|'?kè‰úÙH?`ÓÝâ½"?"¬iÙL1é?x"Šv²U?îò¤5?±U»Ûà¤?†9JU™?ž£0•Jßµ?©MQ€Eø—?®¬=% #?îz"q·Rg?—wù~©?‰ŸÎú¿óL?†óæePñó?¡îÕ#G'¾?'Nuêùï¬?ì~Ö!Š>]?˜ôLÑ;‡Æ?•ïM>òæ?\æs†œQ?¶ÂS!¨*Þ?—	=ÏåAGN4FGL J0112.8+3208¿ê^,dH:=À>ƒâCV—À83È23XóÀ;Äöƒ{á@Ü4d`§¶@<`Ÿ?u¾Ú,?±#™¸"pÃ@üm'ºZ@ÊwàŒGL¿Ö':ÛG¿áÿe:í;Ø¿åú#G,å¿å €sWæq¿êLÞÕãÌÄ¿åÄ|ÁNjAGNfsrq3FGL J0112.8+32074C +31.03?ïßH1òìF?`ü;l–û?Mü0vYe?BªÎOšô?i8Á°Ã'?\ººìÊù?ïç"‡z™_?hDYå9V>?5ïƌð?E"ö­V?f=v˜©?e†áÔ}P?㺓Ô?ƒb;q®a?`jVM#%?gŠ²]ü-º?""¬†–+?'ž{êÕËø?ïûöÄJ¥É?$Q"*¿?Ê?âö]vÂ9>þÑÚÿfßu?<M€tÛ"i?"Ç1¦ù­Î?ï"S¬zqá?'éõϙi?TâjXi?KÔ­ígº¸?ˆNÃ풥?'@ůÁ¶?ﺾƒøŒ]?'SÑæÿ?OW}¤Ï?fb(²Zi†?~¾ó.W©?€=\U6*n?ï^ñ	˜C?¿€wÎ\‰?f{h¹h?rï{Ä`³o?'Rm*Vl?*[cÍ·?ïöóþÙ©?A{5ç?!ßPÄ?DJ¼UÅ?O¸0Ql*?@@˜(§ø{AGN4FGL J0113.1-3553?ïþÝpˆÿÀTß«÷jÀ9Ûà$˜e½À<'4pJ@"{ZqÍ@¯ÎÄô'7?³îހº‹¾?¶ÞGH"íˆ@^á½Ùà@Sòt|(Å¿Ï<í[¸{¿àҟt¤í‹¿ãýDcÝ*¿é oA{P¿è?b`ÈAοïÿ4Þ®÷zAGNfsrq3FGL J0113.0-3554PMN J0113-3551?ïàkC?"ÓS?-˜?G¥¶âk?q~,üw?j'éè¬?e¾?N?ïðÕåTi?cÃðÄÉ-?(Áw=‡Õ?9õĜۛO?[T,q\ív?axŠE2Íÿ?ïpä"÷P?7ï¥q*?u{pºVkZ?'…‹È: ?‰	>צüv?†ß=ÂÍ'b?ïû·¸àÔ
?%±Q՜þ?Óðä¹>Î?l"$¶ß?<;¥IÄ?#ýxï…?ïʃpQ:Ÿ?¬Grëúg?Hsr¸ä…?v–Ù~?w¯Ù",·?©vkSK†°?ïÖ/taѬ?zöæå;&?9D¥ò{†¬?Mr1ŸÆ
?sSûƒÝ-b?y#í1?Â?ï3~Á?";ö{Fó/?GoÒ_+´?†v'!"?"µØOÈüD?"6"?ïõ;_–W_?CÕJÞ©?+5¨$p?ì?Wû?R"Œ,(¾ï?Bˆ3É§AGN4FGL J0113.4+4948?㓘p=kÀ)ÒŸ˜·À8Ùì©&¥À;ºÇply¦@˜ãy·|@^·E|?¦Ñ›¯ô?±™é¾·5@
jÊA¤æ@èæ5?íԗœiW²¿ÜÎQÝr¸¿ã^ö€$}Ž¿ã}FA­¿ãÕ4ûE†¿çä]­Z@¾AGNfsrq3FGL J0113.4+4948S4 0110+49?ïòáTÕU™?H³å)¢×)?!Lªks/ ?ãÊèéÒ?XÀ…´¥?GئÖ?ïï1z½p?jÖ{ÂÜŸ?+§
Ô°|?A
F؁W?^()èM[#?i9fÁ¾›n?ïª '<ÚÒ?{›×X 7?^ãƒMtùa?fC"­¶,?›…¹\<u?wL҅
MÜ?ïõOjnf?85g$á?íÕã2æ«?Ò¼í-KF?S²ýìF(?7)GÂä?ïçíH á?]MÃ7U_?*"úž«?ü‡º_Uu?gV¥'Â#?\hfæOêù?ïÐG›þX?…êš®£[?D샩	Ç?e­›¸‹Q?u>¡"
?ƒ°8bä#?ï?s2|ª?Ú	ºS¤s?d7ÅX­?bøÆüWl·?‹/K©'.?€JÂÉü&n?ïç?ðŽ{Œ?U7§'Ù˜F?/Øø^!—?!X£íFö"?f€5JË?TS§ê6·oAGN4FGL J0113.7+0225¿á¡îÆpàÀMûïÝëÙÀ:h†Úz4zÀ<rû@
faÞÂC@%iF·G?ÅbB¶3¿›y¥ÂÇ»?ÑÞ`þW@@}8ém¿æó0¿ŸÛ¿åNx¾­¥?¿çœÕÃìS{¿ãR&]·Á"¿äÜ¥‡äe¿ïÿù³>†AGNbllUGC 773?ﳧH'?v":ß¾±?P:^vÅ£?@Ûö
K?&¾<߂?u;éîü6š?ïÏk§\¿?už+Â+)>?F=‰Ä×?L…ïšs(?u‰$€¹¶?s ‰ÝkÚß?îÁin?'#Ê:Íç?s»ÜOü¶'?sUØ®ë+?¡i‹ 9nQ?'n'Ÿœ?ïGŽov?r€ƒsš‡?Q&–î÷ ‡?4³8eó?•ûȬºZE?r<—¶A§_?ï1lpZtÚ?‰ÓÜi*š?dçR/TO?X;ÇìÅ?—5‡¯0?Ì¶Ç×ä?ï|I©ê?Ž¹jƒý16?WQ1 ‰ì?c€s5âO?Ž
"Ÿ+?N?Œ—ä©0'#?ì²6óJÿœ?¦D…qí¤?†'dBÖ±€?~`R¥½2?·©[Û'ko?¤'öôKhu?í؜Œ›·à?'-†¢¦E•?j^ßÆ9Ú?X5Á'?°h$h|?÷Û½WCFAGN4FGL J0114.0+6418?î¼®ž'a³?ø£~éÐÀ:&xèI*À;Ëe±Ím@ ëW+5ý@)³(é-?ÅË#ÕGD¸?·£3÷(k?ìOQâJãS@=Šzº0?—p4£ý?ß&Á°¹ò¿âàKd'`˜¿×c§úÛR÷¿ç•¶ë¹÷޿׋²ü;AGNbcuGB6 J0113+6416?ïª Ùz–Z?v²'v+I?8¯DØÍc,?1"~?"²OvtvV?u£O}ÿ"Í?ìÂ[B­	õ?¼'›>µG?Zv~Ï?p½vÅ8–»?¹ƒMÔìx[?»äìź?íÞÀw jP?š†Û:ž˜y?z—ôIY¸?vÝþÃRò4?®ÑebE?™}+}E÷?îÜ+‰	˜I?|Õª<2?hbBSió?Lå¶
è6? ·#HR«Ô?{_ž6év~?ïUýoyVû?‰RZé*ˆ?I)qm$?B22¼"¬?"w'â.D?ˆûx¶éïD?è"}‹FÀ?ÇïlÁÁ£E?pϾêm
ù?‹â÷ Í^?Í+‹Û&=?Ǫ'ñ?ë•ÿHþ*?§1¸÷y?"ª õOð%?G¨Ô]¯?À]XÍÃå?¦Q°¦ðR
?í&€Gc?"ÏÑt¿?ÅKáAYU?k¡Žc2:?µëŠ"Ö?"ˆ"°,AGN4FGL J0114.8+1326?îr.¸*ÀH…S`Ð$pÀ9È=ñÓÀ<"HÏ|ª@%ôx7t6@ÔQ[<f¹?§JdR:	'?eŒQ1 áâ?¿ÝϾï"x@†ª(²ý¿ÜÀêm¬¿àùL`RP¿ão·]yØ´¿Ý×}_§/"¿ã:x øóò¿á5›WߺæAGNbll3FGL J0114.8+1326GB6 J0114+1325?ïöAŸKy?G'q×ëÃÕ?"u)¨î?4ûs>-?Q,ÒÞ?) ?ERöAò0?ïìm®{ W?hXùóvܸ?*²˜-v/Ë?<Tг'?aç(6¸ [?eߋ*éP?ï°x|Ø1Ÿ?xÊ Þ''3?]Ì;¨k?p
1éãÝ?€(Ye8?tISzV?ïî7¥!¦Þ?C´ú—W?0Wm
˜C¬?ç×¾ØÅ?_zڟÇÓ¸?AêåÍoˆ­?ïëM^½ð?`­E¾ë(©?2Ýt
8ºÁ?)5bbË?bVóš×ˆC?_V'8ÏbÕ?ïÂ?K€˜'?€N=Äìa?A+nýʵ?Qšø ¯rR?|º÷
VÂ?~hTR!ì?߂î?'ö´û"jq?`mm—a?o]þAÂ?‹—Â9(<?€*gޑÀd?ïډã»s+?^8*

?Bž9šÉ ?3I«ªAæ?pgG‹š"?[Jìd!$®AGN4FGL J0114.9-3400¿á^¥úrnÕÀT]§°³''À;_»QzÀ<¬zyBáý@!Á\+e‰?üÿéYËM?Á;–7¿ áŸlÂK?ßÚr\"Ô´@j¾—ÕÊ!¿Û2pžÎ¿èÕ?AßHz¿ß‰üÙ´¿â‡Ÿïôð¿Ëáw(Öc?|~Ó"Yú¦AGNbll1RXS J011501.3-340008?ïf{ßZª?»œ¶šz=?1rZ€%õ? Åι«¼æ?'ùâÀ»,Í?»žoN8êz?ïÌRž³^è?{¯ŠMŸÂ?H'w°Nj?VçŠ4Ù?vāÎC"×?x''*Ìg?ïRw‰(?†âNÌé=¡?T×³Á5?`éPï@?"hþ©æ.M?†hýÚÑm?ï˜u'ÜĚ?q«êï'?(3gÛ÷í³?ÎËïóV?‰Í¶[æ?q­øÈg†!?¹†§'?Ÿ
Ñ·³¯?E£:\ÏÍ»?<Ç퉆—?‹Å^ñp(?Ÿ
5II0\?ï™~þÛ	H?‰ª¹#8"?KÿG¨¯¡~?]•øš›û0?‡àKÌà'‡?‡×å³W2?îÇÎ.æa7?5;y'bû?Uì&NZ,?J»r5ŒÃ?¢Ó»ât¶?(¿µä³0?î‡j§¥á?'¨Ž͙?BÎ
™¦¬r??Aø?ðwS?§>cfwp?'À üœAGN4FGL J0115.1+2622¿èwBbÙOÀB~|âÀ;Êön‡À<m|ßýa@8——¶Àq@MíHû?Ô3ÿ
z¿¬¨PÁŽ€6?åü·ÁLæã@
4rIs'r¿än?Ƕ¿²]¨@•5K¿é¿¥Ò.¿ÖKIàâi¿×*Â+A¿ðAGNbcu1RXS J011451.8+262337?ïÞoÞ4S?uÓ.vò?3)^gœn?3iN6:—à?o†'‹Q?täAŽbÕG?ïÜMfmÐÇ?o¿[þLj?8%Å{'®?EÚ¡Ä%™?pVðˆ‡?l3ï}x\?ïaXR°Ç?‹ŸÒRNª©?Wá'èrª?bxoîÉy?'V݃êŠí?Šë'*ç4?ïÐy«S?XoNí¥ì­?-]D˜‹»;?r‡tÒO?vØ@Yõ‡\?XBi¦F¯?ïÍTï="?u3ßJ?A/šàA*?;g'Ñà?w/¥Ÿ`QÕ?t5>ÊñÎ`?9áçÖ?‰'yV(?JE-9»F|?_'	'ž­f?‰už»ã±?‡+H:þÄò?îý¸Œàl?§´'!
?`VEs´þ?eDŒl¢z?ž>%ΝfÁ?N	'ô§?ïbQ¢p>?y¶}CçOI?J{k9aÔ1?>˜ÅB€Cö?'áðV†øÂ?yl&LÐ}-AGN4FGL J0115.1-0129¿Í¶:'BÕ_ÀOßbb˧3À:î¯÷ªÀ<7mƒ'˜@h€•'¢)@¶';‡?¾`¿øì?¹—´<25\?ò:e;Ãûm@6ƍ?îQB‰hI¿äµ€r'¿ë)ºy
2¿ìµÀÁ¦©¿ï'›??ï;-ÇüƒAGNfsrqPKS 0112-017?ï÷.uDŒ?P}"o?"™Ð a"?!K)¾ª$?NäÒ½ÝdŠ?Nñ¹Ùû"?ïÔÇ(YK²?w¡!·+™?Ha,Òª?XÛÔ­c÷[?rF[Dyv?s{&«R6(?ïµ±úÛË:?pìv&ø
U?Ziù?VAƒ`ý±?~¦(Z&'?oŸcéü‹ì?ïã½£¨Õæ?M¼,€N?C5x~Ñ?)O´	àáE?g•f?J‹°Þ*@×?ïïIäÐy«?\2ªý(?0Ëh?(ÕTÓU?]9\ApJ?[B–¦À¶£?ï'J‡…o?'¾°•¹¯?\¡E¡aœ?y·ÎçBê—?‡Ù,~ö?‹:݀â9?ï"èg]k?{ï¯qÆ%?cÁn?d?b@ÙËÎ*?‰ÕŠ" ¼l?x¨Ø=šF?ï—R³?s….ê*
?b ²ô¯K?Sw¿ßL$?…ƒzéî*F?q*æÅ$AGN4FGL J0115.6+0356¿ê¹¶éûJ¨ÀM0—á2µ_À8ûá÷|þÀ;ø­•Ïà~@a$H¸@Go*ZG?¬
é½ôAÜ?²"†Òeh@X>»&²@\ìj!¿äa³'¿Ù®=•ŒÄŸ¿á1QFC±0¿à†&˜ðý¿æüÁâc¿á1´âf'AGNbll3FGL J0115.7+0356PMN J0115+0356?數Sº«ý?8qŽh{?R"Á/U—?UçÆ%#] ?"CùÕ¸?ŒÖ'¶Ê¤K?ï‰Õ	}?ž3¼~Žœ?hO@Uí´¯?·@ݹ"?‡¦:˜«}µ?—Ëm2O¶á?ï,Dt¬­Ñ?'jÎ|¤q?ný\?N¨?x_o]¥1†?–—Åâ€pÜ?ö0õöyµ?îâ6Xµ?{ëõDWÎ>?{g› S›×?_2àÈnª?œßVí@˜s?x®{ӗ¹?ï2èò6,§?—,í-qP›?iGCÜ.Ü»?f&{†]x"?–yùEo®‹?•î¬4j°?î''Ý6ì?³ª4UùÛ?†!xOæÕß?£ÇÑ!†' ?¡e$\9Ì?©‰!ßN­?îjd¤^2?œ«YÒL¦?wuuëÜ^?{ð×gã?¦kͱÿ?›p­Ï÷ô?ívŸ,O7?–뜡!R?isdHC?{r"Õ=i?°]Ø3+}<?"žÝÀm¡AGN4FGL J0115.8+2519¿à㳪M,ÀB›–À8¥´B'KÇÀ;¶Î¬ Ý[@Kn	È֞?þ¬*˅¤ð?£‹`-¸±?JïË
d?«*JX…@ãLÓi©¿Ô åΑ¿âyDÅ+áY—K
À¿ÛJÝÿz)¿Ù²†eà/¿Ý"o@ª•AGNbll3FGL J0115.8+2519RX J0115.7+2519?ïôŸVÇâØ?\f¿;¼‡?T[}iÐ?ÜÊÓ!\?UL»'Èl?[¸8½J­?ïî"@AÂ?d.˄u2™?%Ì$Óa›-?7Ò_5ÀT?`žªD  ?b²èÈõ]?ïÔà±Iþ?"xû+lÜ?S³ÒæNvƒ?^7™
öj?œª&¶vi×?"ñÏH?ïø¬Ÿû?3oeõ'µè>õ"$—¯šŸ>ãÃüaX"?L£,È9"ü?3"='`Þ
?ïð'b©˜?X	n›ðˆ'?"jò™enP?õðF
¡C?]c‡=Q??W)A‹ÉHõ?ï A1+O?† t?á?8{ÇMó	ù?N=dM7Ìø?}("úOÂ?…çI¬šé?îà-‹9À§?–\÷ôîª?W-š0…p?búPÀr?¡Cº~'a"?–À(K9?ïïéýŠ.í?OT¤‹ Õ?€NÃ?êµ>ü¨ýö?_hý¡M
?Në;èçôAGN4FGL J0116.0-1136?ïÿ£NײÀR\/ƒ{J#À9Aª>-À<?¯à,ûâ@gÈ;B¡@©½R†?©!="±l?­[Žœ•Ÿ@¢Z2{@Êæºßr?›­5F¢•…¿â"Üöæ{Ê¿æ·hí)c§¿ãY`>.8ø¿æ¿Zž\!¿ïÿZªÕ+AGNfsrq3FGL J0116.0-1134PKS 0113-118?ïÞ-ÛÂ?}ш†ìT½?1VÔÔ]?9ÕSDdµ?oÄhF²¹H?|ûe
æ:?ïòIý?beçÌëž$?%Ó`|+?8/ÆîKŠe?Y–¦Â?`\JŽXš¹?ï'ó8áã?‰‹çH[àè?tÝ,È3U°?'6õúád·?"Ô›e[*q?=©çÄ¿?ïý-Ù	ϕ?Gn>ÈC?	ÊÔ2çHb>ôËÔtºŒ"?3WÛHZÃÛ?iNõã3?ïáO›s¹`?jü¬mĚ?2¹tl9Ü?0ç#ÿʜ?lY5Ø'i"?ipـ:ô?ïÕê¾ÒŽ?}»´×y­M?9mÊ'ücô?N:*–Ú?stç{c?{Ą
Z†½?ïKá"9?Œ#¨é¨+¬?w68±¯]?‰;»µ}Ç?ÃŽì‰¯?†²^Ô¥?ïù'{_i>?7â-W_6? ƒ¢ÿ
Ë	?Ûôz06V?E™)&v æ?5¯Žg>wAGN4FGL J0116.0-2745?àÊl9(ÀU ÃLŠÆÀ:ýayWÀ<Ÿ\>Å7­@!R'È>ô?ûšîcŠ	?͏t|©Ÿ?¾‰œKz§¼?ï
¾ßÏ3@" fQïýÁ̾Š?ïåt™/¿È"%Ú/5ù¿á½>!£¿¿Ø¥{úø.O¿ÔÁ*AÇöyAGNbll3FGL J0116.2-27441RXS J011555.6-274428?ïÖíݓ™z?‹WRÔ¦?55Er'°¼?Nµ,f©ù´?s5¼æRíQ?‰¥I#€$ã?ïá5ü€'?t?ŽZ~*B?5FusÚnt?Dn(ѐ֌?l!5
A?rŒÌQˆÐø?ï"4°5èD?ƒ*‡ÉP¬?Pê'Oöõ'?9´ðFdÿø?ŒÕå¨+?ƒsÒ­Zð?ï³åP.õ?a3'â" –?<kÜ7‹dk?&'£Vöªs?'#M‹G>?ad֑m5?ïÂ]'ÅS ?–8Ž‰<¡"?AÜÕA˜¾É?L•Ft	°?|•œ†ÌI?•Ç¼½l#î?ï°A±{7¯?ˆ	ÿl¹ ?E²*.Å?SÁÝhÚï?'"jÜEÿQ?†ÛP¶5bŒ?ï"¬0†@Ý?*ßã¼
É?Vk†~?O;|¡¦·!?šBaÙ¡·ï?ŒŒçÜ'½?ïG¡Öõf?~+ÄEëúÁ?Eæ©2?<]Ȕ›[?–\"öUþ?~»Pü,nAGN4FGL J0116.2-6153¿êGyCbÖ9ÀK~r\=îxÀ:}ç&f¿À<š ]Øù+@ 3^(6Ö?üÈÈ@vÕ?»UÖ&"?´zڀƒaä?úcˆÕü÷?ýNá9–O¿ïó?']<?Ï\°¸¸Ä¿Î3BL«ª=¿áãyí+çå¿ÓQ‰_²¿âyUn"AGNbll3FGL J0116.3-6153SUMSS J011619-615343?ïÊN‡nì?k 
Šê?C·ÝýµS??7ágö7.x?x{]Z˜£?jf\ÀŸ;Ë?ï³úp‰!?}ç
J¥å?U2åãM²…?WŸYÚP"?€[4=#–?z1[٣ׁ?ïvªa›"?v»ÃQÜ;4?b/œöo?aÔÝ7·%?É¡øwp[?sÙR&ËiH?îåPW8ÿ"?z9u­"D·?o™3"ÃK8?V3¾Üé·T?ŸbΨÛ[$?xþ‡À`PJ?ï|³–C?|õb¶b6?\'%K.øŸ?Rò]Lƒ³¡?ˆŽŽdŒ3?zžF¢´Éî?ï#ë'4Ëd?™9—Àqk?f!wüÄ?nmý@Í®?˜®é†»ñ?—.c¡­=?ï#ã£Â¬?"jjÖ-`Æ?l^óÌ1?jÛn'\Y­?š¥s¯]?'—Jã°±?íDÄô¢e?"ö(ã9{?€å%Åé‹?q­yí'È?³½3ºˆË?"h…ãIßõAGN4FGL J0116.5-2812?ä"¬2sxÀUÎÙ‡+À;Zm]ÑloÀ<šVHáñ!@õ^*Ü#@ƒlØ?Æwe'+O¿¯]ÃT¨ù´?ãüµþT.U@ÆÞþ}Ÿ?åɛ?-±¿çbz¿å"u'ÊIe¿äê•ÀF+³¿Üãa¹®b¿á~ÁqN÷µAGNbll1RXS J011637.7-281146?ï׫v)Â?d*Ág%æ?8üŒ°ƒi?'õÎaHãZ?ráár¨im?c›…|Z´?ïÇ4£åf»?}XiS®?OËK±û¶/?YøjÛ£?xlDŽ‡½-?x¦©–t¢?ïf$wÐ5?È4/‡*?]ÂQÿüP?W½mh¡º?'_XEµm•?@2(%ù?ï· Ü·¢?eoÙ®fî?4••eƒ^?!b>±?sJ˜
€?ef§ÍŽ'œ?ï©À°ñ?u'¯îc?KüLQ•~º??U­#Ë|??ƒü?(}Û?t|WÓ÷D?I"?'É€+]?Wô¿B>é?e†Pün¾`?ŒV•ÔaBo?1c3¨Ñ?îé+"Щs?ŒX¼Üf^?hÿÖacƒÆ?g3N¥-è?Ÿº'ž¹Ð,?‹&–¨ß™?îû[ö Û­?†öC?z&?P¿)oëÃY?FDø²e?ŸˆŽ™V?†j/5ÝAGN4FGL J0116.5-3046¿ï˜33øļÀTÙp÷¹àaÀ:üd^NiðÀ<¦ù)L)¤@»Ç{)@˜jßqë?Íåw©ïÏ?ÃD͏jk¯?ò\T)Md@ˆ|ñm@?ívѧR¿ã"Q´þ¿æ¾ç0ü!N¿ïþŸ½Êü=¿íjUéŸì?ì0…ÔÀ·AGNfsrqPKS 0113-310?îq*[U?Éc€ÿ€"?¦é°DlEÂ?É}1(?pP*·O?t"émÉ/?ïs^ÔC0#?"iJ ?q¾+§:?€&›pÄnF?Š£ëð
¡?ŒR9ß3ÿ?îàñÅ)ÀC?'›Ü{€¡?|C…6?$ÒÏp˜%?œ½¶gš-?P§üø}o?ï™cŒJb?j
Ѻÿ71?^—г5Ù?G¸ù²9GÒ?…Ô"Çú+à?gîÝóڐ?ï¡2OB]?˜h†O…'^?h"ÃRºâ?•¹@Ù
?³V	É×?‡H2‹?îÖ,_·ÿ?§£äR"Ø?€"H´\8?"Þ¡èF?œðϬQ˜? ¯MA¨?îOùÈ-€Â?—5¦ÃX?"ݱ–Ñ?…/Bkh‹?¥ý¢	ƒ +?"Ä
d§›?î ©²…<¯?jZLàU?tO9aŽ¦?gŠ3Uh?£k€î²7¼?‹ Á
‰·HAGN4FGL J0117.5-2442¿í\ÏcÕèTÀT颣Y6À;ÁV¶JªÀ<ïCœ7Ì@!W"È×Ê­?ñøDIÛì?é!—c•?ބwžr{?ñ+k…L?ý;IÚ¿~±¿'¢Ïù'Ñ¿éôöí1Ç"¿ïí	þ±vZ?Ñh=¿çTbøóœD¿Öà¤E9¸AGNbll1RXS J011746.6-244329?ïaÊfÚÄK?""	Þ©ƒ?Rg1#xÔø?I~PiE ƒ?' @ÚôC?"UêVñ4}?ïÇÏkì`?M·sjJ?P8¨}¹Œ?_¼-Ô·ÅY?x
 f91Z?}BŊ«ÅŒ?í'=¿u˜«?¢â†¿N?wP¡Åmv?}¤»LÐõÈ?²ìú™Ø'?¢­nG7Je?ïIyäÈ?†¯'r ?;ë/jX?A̍þØýû?–a'8£¿Ë?†t¿õ—Õ?ï#)ž3÷?š0A)÷û?iƒ1ڌã²?yÞ7u8™€?˜jyIÊ·?˜³7¨,?ïo,s¯é?¡›N\{ÎO?i¢¼}&JÝ?•ÉV˓½?Ì3ÿô²é?šðM*aDÂ?ìñé}mÐ#?¦˜:Èù–?ty+=…?zFñ£hG?·/\ƒÌnQ?¦)B"ø#?îRÚ¼_Ó`?£¶'"¥†:?HÅêh'³E?``Ÿ'ß¿S?ªo<'œ>(?£¬3¾2AGN4FGL J0117.8-2109?ïÞU¹®@ÀTa¯ž¾œˆÀ9lszKÀ;æK!JÓ@ÛBV¼¥7@¨¾e*ý?¶ú³åË z?½j°£vg@ý¾`l@½X~qJ?ïú"Àā¿×ÅÑZûú¿ås^ ò"Ü¿å锹`~¿æåªda¿ïú)âQ™PAGNfsrq3FGL J0117.8-2113PKS 0115-214?ï÷&üÝÐo?E1"xH‡?xÅí°™•?oZúEåß?O´òÏ>k¦?D—L?ç?ïéÚ¼FO?n«ÕFÄm?1ÃJs!?COã:CÄ?dË6̧,?kCàX["?ïÅõÃ6?'îúZ?ic_†xŸ?p`°Ò—ÓK?‰5ª¸¤?ÃÉñã¡?ïÓÙéÀÎg?VvîHócå?C€`ÕY@•?,Êá¨Óï?s¢ÿtæy?U¨l¹p]c?ïôH >	·?M^% ½N?- þž?(Wæ+EÞ¿?SËë."?IŸ£Œ6ž?ïÉ9+3¤6?€²‰Ò˜¾?CŠšççL?X8º¬Êˆ?xòŸ]?~BÄØX"?ï.‡ ‰ý?Œ@äÝËÞÌ?u:^ÝÈS?y}§!e8?"ÇÍPÙ ë?ˆ#VìÒ¥?ïˆ6'ّ?tìÖWEz?\lìþ £\?I0ŸjZ£?Šd¾Ç{}?taÚhQZ3AGN4FGL J0118.7-0848?ä¿B0ã3ÀQ¤Åm\ú­À:nÀ<~lê&3@MùÛùz@ÐÛä—Å?Ï1æÂlK®?Ò\'þw•@ùCM\ª@	Q¬«5x¿©È&ÊÅ
·¿æô¼U…ÿåë澚¨¿íb(E¿ïÿÙi"A'¿ã.<=óÖ|AGNbcuAT20G J011844-085058?ï拿ˆ¸î?d\'ÔXÛ?DWz,à¯Û?<	=đw'?d^aÒ[k±?bA5Wå??!g?…Ö¯-zY?cš‹ÿù…?i©ø@ÖÐU?'w<°á
?YÀä'܏?ï1rHa~?Áu'_Ł?n`ÚEŠ¾?r'˜`ˆz¾?–´úçõð?øD£1è?ï‹jHëx¬?iÂm…m?gUÚa9É?K&"ILÕ?‡b˜D'¨¥?g|oóq?ï±°ùKt·?€ª+‡GÇ?X<€l׃²?U[óuGõ¡?€Œ1¥·-­?~·3¯ñ$?îýÀd<H?¡\ÞÎéí?zðmFš/?í}¡Ša•?™¡,¦uKç?™ÉÉüҒÎ?N	:?—³ñŽeC?qýÈV<@?vs	YO?¢f²"T?–/¡LN3Ö?îò‰Ië1?‹m#p§ÅÈ?#ºG¯'?psÖÊÓ&œ?£·èÜoN?‰b͆"^·AGN4FGL J0118.9-2141¿êckWÀTnð¹À89¼R+EÿÀ;ƒ|@Ã@æ-Lê@œIwB?‡B÷Bä?·dD"@;p@Ú»£@P;\Í`q¿Äy
t­¿â<i"‰G¿äÄFwÜ¿â¡fµN+¿è6;ÏÆ|¿èéQ'©"AGNfsrq3FGL J0118.8-2142PKS 0116-219?ïž88Å]1?µfÍà
PÃ?[©ŽmG#?ˆŸUs¹…ÿ?"ü¿ódU?²{pYqoá?ï…üšßƒ¢?Ÿ@Œâp?e"+ƒ*A?…̬Þ°J?‰Îd<ð•?™ûAKÇ 2?ï‰t†BWq?‹Ÿ¹Ù{?s[‰Œô¦?>Ç]n'|?ƒõº–µS?"
™Œ&Á?ïMø̸ˆ{?y!"·!%Õ?jÇÀJ"Ã?W's ºÿ?'çîbßùC?v0ÒÀŠ©Ò?ï§iÖ³U'?®þÎÏâ?Lí÷5–?QnË~ßÕ ?"VªëS[)?­¬Hm¹M?îù.^P?±f&QWÉ?€b	¹ü"?ªHŸ‡îl?˜«UW'¿?£5/¡S-l?ï`þóe'×?\÷ý¨ø?|"E9\Š?ƒöb"Wr?‰v g¶j?‡¸-7Ù{«?îàMÞX?"É7}+
+?"ËÇ8Ã&?uCr"ž½X?ª=4‡6?"Skä‰ëAGN4FGL J0119.0-1458?Ç'(è¶bÀS†YJôñÀ:I£–ržÀ<V>Eµì¶@ {ßaúÆÛ?úgJ&"¿??Úl'p‡R?¾ÀRëà8d?þ1Ó·¢™@ÛEPl)?ï÷Ÿnc‹¿å2GzèÔj¿Ý¾6|=é¿Ñߢ'fŸ¿Û¬ß\‰É¿âÊÕFEAGNbll3FGL J0118.9-14571RXS J011905.4-145906?ï"
ˆ'€é?­Î7<ú~®?pìÅõôâ‹?­ñCF=?'†úñ#ts?v]V¦Œ''?ïÎséºL?vôÿïmò?J-ÞEŞT?UžÌÚٞ?u³
)1Ñ+?s+ ¢3?ï<|yù?…áíћ?c9ÍŠéU?bhÞ¹ÿØ¢?–¶Æh>4?"ŒÒÿF?îõî[è´	?uÉ]9h—É?\?·?çµ}?A¬8é«=?Ÿ~9þ‡?uBˆ W†Í?ïOŸ".O?Št&ŸO[Ë?c1j@ȕƒ?oݝÈ?"¥â/éo?ˆx¶"'Ê"?åYÐE?éa"*Õþ?X ð©ãv,?cYˆG5?‹×¨…á$?Œ	-/ òø?î(>x"Cø?˜‹â¡ËA\?pÑÒåOƒ?l´ÈèS?«aÞUq?˜h{ œ?íU*yÚb?'vM-="?m,".ßà%?[á=vEë?´mJÂW93?'7ŽfԃAGN4FGL J0119.4-5354?ŽM·Ý–7ÀO[ñ•1äÀ:ÙܲÀ<µm¿öûu@×o'yÇ@Â/BêÊ?À‡‰v¶Àœ¿¨§q@˜y?è[x¦@Y
\J?ÄB§Yö–u¿éqmŒ¿äüÅd"¿¿ßD˜¶DË¿ïóO]`XZ?âM‡rO¨µAGNbcuPKS 0117-542?ïÊ. hš?€%˜i8•Ø?UFQn?ÍB?\ör@Aí?u—[""?yÏd5ä?ïÊ&oVX?xÎ\Q_"5?O36Òé¶+?Wrœf"?wŽÝÑsz?t׿"*?ï]R<I²?ƒh¥j¼?kßcQ¯Ý??liØüzù<?ÙÌך?í³Ž˜¢¹?ïÇPrD|B?Y؏McSÃ?V¥;áK??yÙ
Å|?v®wéšß§?W ½/5û¢?ïu|o??ŠE°pX?j¼aú¤%?cmÚ¤¸Q?Œ	ȕUsA?‡<ÿLÂI"?ïpAèÇn?'讥{l`?`G9ÿü?jÊS-P'?ëô
3î?áÐ6†Z?îöÔ4öù?‰¬Êz—^?pw
ª©8?g³kt?¶±2Ó?‡üÂDïÌ?ïCù1.Ì?~Ó¦§?rç&Q7Ôý?d…9ÆæOö?'ÇA¸ÿ]?z8/ŠÌ=AGN4FGL J0119.6+4158¿îÑNµ«ÚÀ4"ó#x«
À;DÛ;$™<À<¥ˆI=‹@¾½º`8¥@Ÿ°ºG?Ð'L†@?È¿ˆ–'ýC?û®oÜV?þC,»–ï?ï= "Ds¿¯´Ê!¡»Q¿é6†…ÀŸ¿Ü»õy"@"¿í5Á¸œ" ¿ïÿX¥³ƒPAGNbll2MASX J01200274+4200139?@éÃí?¡¾¼úØßç?ˆ%¾ŒŠjç?"B[öõ
? +ŒPÔÛn?› NA;Ÿ?îìv˹Qp?ž8("yu¹?†ŒrEn~?«Ž*þñ?—+ØJ ¹?"Ý«á'ŸB?î³õËs±S?'RÕ%f
?"þÌkm?ƒX¨Æág?Ÿ8Ç-âó?Ž}ëk²üM?ìÿV×t"?'
¤öNc? ö^G°"?€p`uk¨ú?¯ì3eN?c)•Ü'ì?íýköÎ?¢ï'T9°S?"t¾"9Ôñ?'O,y_ÜA?¥îïRì?Poƒ2´?ìØä»´,?²É6èµ¼? Wó@…Õ?¦!ã['ÓG?±-®(MÐ8?ªŸ^"̽ñ?íãÃ%{‡?ŸgŸ?ƒ ?bi¶åËE?´«•­l?©'˜ÉeM?˜Á¡ž0?ç'×I8¿J?§ûZ^-Md?µaÛL5pw?CŠÛ6¿?ÇCµ4]]\?¨cP4pPAGN4FGL J0119.9+4053¿ïëá©Ó¤À5¨¡œZÀ;œqÀ6¼UÀ<ØÐÜüŹ@ ÄLˊ­?þº"Àõ(6?Ø:ú݁O÷?мXáB¥—?ú*…ʯ¼@`ô)2(q?íÜã›EkD¿±uWELå¿Ûç};?¿Òuác\ƪ¿åÙþí[c¿ïô ~$É
AGNbcuCRATES J012018+405314?ï¦SþÒ$ó?°YÍÓgXš?I+I2©?Jð@gÞL?"ØKÃéG"?°Z7ê¡Õ?ïo£c>`/?Œúâ¹çûy?n•ŸÔ¼k?v"Î^1a?Œq¿.*j?†z×(ö¼?ï5²©Wt(?‰ ZN¼7?r«… ?t÷]õt¥à?"È#¥©?…ò÷§î{[?î's©´³•?§ÚÂ(»?yÚfßY®?`•AðI?£"uE&{?€É¸¬j'×?ï¶Á	õø?qC7½O?[?Ú^!r½?T»x¯Ó?}τM/EV?n<šZtô?îw<oûn)?¥Dœó?'Ù"¤?"OÊR%?£Õ×þÓ0ô?¡Z#؏?îÄ$SÀÜ?'¶hBšÀq?|œˆz !E?ÉÍ5tÎV? *)¼jh¤?Ž–¾²}¢4?ìµØ¥¯8?Ÿºj'Ǩ?‡C~›@­?z,4Z]k+?¼òhʑ*­?žôAj_m™AGN4FGL J0120.4-2701?ïý(‰…-ÀT⹩çÀ8dµ—&À;YАä¿@øŠë«à?ý#8ê,Y?âWùf2å?ª²³_ؤ@ñ¡˜kœ@§é2Þúw?ïýŽ5¸H±¿ÙCSy¿Þ@áDž»¿ÚtZe&Jm¿âXQ€%TM¿Ü˜‹<3·èAGNbll3FGL J0120.4-2700PKS 0118-272?ï´UìŠq!?‰æ æˆ?@¯–R‰²?H®ÃBã ¨?ß‹ƒ½Ís?‡ö]ŒD"Ð?î°1'rÐF?´»ükDq?q-ïnþ¥?Œ¬ù¼Ï<?¢×)÷9 Í?³ëÙ¿ÒÒñ?ï$¨n§09?•,õ±'jÉ?~ÚS7¨jo?ˆ8î¤õ?"´]ZÈ$Q?ÿ3ish?sSgd?ˆŒ•Öꨘ?l¬ø¸K•?S—L;-¯¼?£I?l°
?ˆ^vbDß&?ï`m՛}?"-øhÁf?M1_ù=ib?SXU°Íô?"§@Ú?'¯¨j;õ?í:·[ö
?Ä7Ðòv?†"‹Î&?°y89Ó?³XT—eC?Â}ÉœÔ{?îÅöc
d?–,bü§ðo?LŸ ™?…‹'¸"®?ŸnµæZ?"¿ 'O§½?í¸Ç‡=¡v?œ|ã@ܳ?wD蚏?g¦eŸû?°ÁÒãÉ/ã?œƒµÎûȅAGN4FGL J0121.7+5153¿ÛÈEÓb¬âÀ%dí0µªÀ;'³ S\žÀ<ˆ §ªÔU@"€±ˆx´ó?úï'åJr?ˆZ!´†?À"ÈVñSj?÷V%¾@Ø!ÈýŠZ¿ïÿÀ	oëJ¿ïuÞ©n#?ïÿXJ¿¼sîdL/Ù¿ç
çIOÕ*?"™N›Ÿ´AGNbcu3FGL J0121.7+51542MASS J01213367+5155520?î†vÙ±?£¥Ò‰'(?Cµ\V?:­yó2F?§I¾91#?£""èô†?ìf–Ø9§?½BfÊíØ?mÆdøÚ÷?{\jðQ÷Å?»ßKŽuñ?¼¤ˆ˜·¿?îCD HþT?—¼]jK?fz¢ÜW!?j(<×Æ(Ú?ªdÐÂOÆ?–ñèg'Ä?í,Íz¿[?"X&{¢ŠD?pµž6|2ê?bG³L
?µŽ:E'2x?"TØ·v*R?íAŸ)¦l'?°…ìä O?Q¬ß'8•?I*%ÎK6?µ¬S5«4V?°x§qù‹?çìµf—?ÊÑØ^5b?qoÔmÑC?|õ[æ }?ÏÁ­›Õx?ÊɅ˜cl??ìY÷:½á?¦z´yŠS­?rKâ>;4?pÏ©÷ŽÛ?¼"*;_I?¦3Ö:`ƒ?è8BÑ¿?¬=ZNa)>?'®ÕÙLuA?üøY²"¸?̔0l7p?¬c´':ÌýAGN4FGL J0121.8-3916?æ
"È=`ÀSyB=KÀ:¤ù8e¢À<›"´W‹@ "]8??ý"6÷
7?À—ða§dÞ?µ†
`:Ó;?öàÄn&N@qÝn°ŒÐ¿Öp¨ÿ¾Ç¿¥†K3/,¿Û¶\þˆ±•¿Ù›¨B›†¿æ'ø»h {?qs™;*AGNbll3FGL J0121.8-3917NVSS J012152-391547?ïïÑÀbÂS?JE]«eè?0ÖUÿŠ‹>?љŽ€?\&éÜ!³j?HA
Yarš?ïØø;‡âÚ?rBÀ0
?A™Š+š¿?IðúÀ¾?qP°áý"?p ½Ñ»€À?ïšãd؋Œ?iÍþÔÈuû?YÕz•ÒJŸ?Un†½L'?†wt»Å?eEs¢È?ï"(çˆm€?b¿&Möó²?W§Ã…}¼D?<%WÀôÍ?ˆÍ°LŽy?a¶ØGíèñ?ïàVâ×¤?`êâ‰b˜?BזƠñô?3
&qþ?jó7Ÿpt?_úíî™Éë?ïŠo–÷å?‹.ù¶¼tx?Xô`ŽÜä^?lDž=3ç_?Š_Ø|Ð'?ˆh?¦Öet?ïUìçۂ-?xzø=ñ¬›?bªÒ^?Qº4L'E?"m¦01Ê?v%!-Š?îï ¯€?}'֝|ÆY?jIŸåÇÈ<?Wˆß(¸ê?žÃ'æ®?|CN=¸ÊAGN4FGL J0122.1-3004?íï»ÀT©Ù¾L×IÀ;ä¨+,ÔÀ<ì·/¡®@#%oÑ@?÷jðSº'8@m}aT®®?«ßXVÍ?þú¢ Í¿¿ÎŒm?îÀÎۚƿéX•";"+¿áW7T*#À?™Á]=¯?ÄÙRíÞ5AGNbcu1RXS J012203.6-300507?ï`Ô¡àîu?¢x˜úڞ"?'*²ñv.?¡pÚ7lö?… $•dw?‡Lʊ²ˆï?戮t0÷?›Êâ~õ/k?h_U6NÔ?ŽEt&¹?€¢Ìq%é?'íWêt=ð?íMòÏôR*?¤P¦		V%?xôº³Œã<?"ú2Θۭ?´Õ[š8?£ Òjgõ)?ï?˜Û?§ßôðøé?
)Çá d?: O¸Ùó/?—ÿ诶¤]?§ÓØ=pY?ïy#yç;?Œm'Fò?svº<–z&?ˆìzPÎۍ?‡ûⶄf ?ƒs6Nâ¹?îïæb¨ŸO?¼ZÁR×O?‡UÁ䢓?²}Ǔ6…?–sˆÏ!.Ý?¯Cy°B?íàž am?š2›	Šm?iÍHË[j­?tyæ d?°, µ×7Á?™èÞÊQýŒ?îºÒ¤R/?Å t>Á0â?$=®Ú­¡z?Z}UY˜?¯°+Nþ?ŝÜðíy§AGN4FGL J0123.1+3421¿›ê€ÎçGÀ<†Â&€À:"Ž;—…ÃÀ<hÉÒ*Û@!¢Ÿ.ÙÝ,?ú~V²"<c?Àì²nì?œHÿ´øè?ßøüLl?@"dQ›©¿ìb>ƒÉM¼?ÐÛZV¢¿é̒ë)¯&¿™
?þÑ4¿ÒS^a_@'¿Ðg\…'ûAGNbll3FGL J0122.8+34231ES 0120+340?︑*'ñ?†ñ…ž"??ÃõRDøÛ?>&"£Í½†?€ÝœDî?…†ßÓpÈ?ïâАŒæ¿?ló*o@ZÞ?1åþڝ$?>'à€ÙJ?jò¯p¬¡š?j²ä'¿÷Y?ï>»…/\í?…ÐlG.›R?[¡ýÛÂÇ?aHö#íIâ?–nvt3U-?…"<"ö-?ïžzVtß?e
ó9ôD—?BÿÅ«S'?,ËÈåûñ?‡1ƒSÞ®´?dÞáò­ÂÖ?ïŒ1:ê"?…äk'ñ‰?OñDM²?Gqi~m{Þ?Šô/Ø5?"øb9Ìx–?ï•ÅŠ@é³?"Þ…šç«?G43'ù$?Xµ4
ŽÆL?‰Z(´aî?ƒxômX¨£?î~^v=Ü?"Ã:S˜@o?aõò3Y`Ô?a^—j‹S?¦ú¹{(˜º?"'vÁ{«Š?îï¹Ïwª?'ú_ÖÐ(?ZU
`C8?N@LdÛÔ? 1ºLõ?'ÏH³¾*AGN4FGL J0123.7-2311¿ßJ3æózÈÀTlÎþÖ4UÀ9ÊR:_w_À<-S±Wü@@ àÚu×È?ýmºßd?²'ØŸ¾Ì¯?˜™ظÏ{?è¹Nª@ø/Ó¯¿ð?ð¿Ü]aÚæk¿ÝI|`Mȋ¿àB¦¾EJ¿Ê¡½?6.AGNbll3FGL J0123.7-23121RXS J012338.2-231100?ïæŽpªÉ?_içËcê®?9ÆÖ€áH?2XzâF}è?f9
‰ƒ
q?\×t±ƒ?ïåøq°
?r	w;ž?88]=?F[Ç®pªÌ?göM{³?pIº"lÐ?ïX=wôr?‹¨#¯
.?y¨¡ËŸ'?ƒÀt°É9"?jM¯=ù=?'YJE\Ï9?ï"wJS$.?h—éR(ì?Rv"ò
¾ ?9soOB§u?ˆÓ\ÆÅð¼?fË;ƶM{?ïÒyÜ(Ï?n	Qºõ?Míôöý?H9­"ž[?sò
/?kS½z€?ïµMNèEy?"2ùoÌ¥b?DÚªISù?T±äÂŒ?_®†È?ƒûÄc÷?ïÑKY?'ƒ"u%?tÀ9gv?~Ø©ÑäÓ?™Õ³W./Ö?[Dͤ?ï"&:Ò8ò?€‹B6ŠQ?bzNÌ&Ò?Rð&\úƟ?™kîÄ!
D?H!´,ÇAGN4FGL J0124.8-0625?ã62C@"æÀPõ7óŒT7À:"t•À<Œ›'8S@[ÅßȨ@'tý¾?Á¾«·ShÞ?¯Z"|ýŠ8?çi%}½ðç@ž•Ök‡
¿è[#aÙ丿䙅½nµë¿ãeØ!Ëå¿â²tý¾¿à}¯XGÀ¿ìÏñ¿öO¨AGNbll3FGL J0125.2-0627PMN J0124-0624?ïú8M××Ë?0°´ë?ºÂÔӉ'?NêpÖ3®?Cçp#Ž#·?.ðW
@?ïò(¡bž?bñ%ò*óÕ?%÷[ú?8Ô¡4۟ú?Xúÿ>©Óâ?`ùž¶Õ»?ïÊöþq?_"*?Ôa?L¢}j{ž?3÷k8Ð÷Ý?vð1$©?]š%ð?ïñÿ«éŸ¹?8ÀŸÍ3åE?õw…3Œ'>ÿ³ ˆ¢Õ?ZPSÕ ?8UžÓ«?ïõžÂù9g?A)'öv™?*‹ŠM³.?d
ͪâí?Qq	¦øä??"Ëñ(S:?ïÏ]ãàå‰?{ýB&¾JF?7õ½Êø‡-?LY{ë'À?vѲKT"Â?z]'"‰,Ä?ï¬@åÇß?j®Q¶"á?TØX…uõÎ?B2g.g¢?'Tô¶7?u?h ³BþÓh?ïڀÍÜÜ?X®£°3è?.‡A±`¤?!7ª
'?qË}ž'¨?XNqو[RAGN4FGL J0125.3-2548¿æÄ{'ûù>ÀT'†@ €À9Û7ƒ$OÀ<wÎaøBœ@NX"¿åß@&¸0]•Ý?¶Økš,?µfmrIHž?ýS
3_¨Ý@	Ò<m™‹'?ïšáBO°Â¿áŠ6ðW'¿à¢ªßè'¿âìeïH"¿é.xMïw¿ïþ¾P¤]AGNbll3FGL J0125.4-2548PKS 0122-260?ïéSØ3!.?Teݖ$ðQ?<=M?.…5Åøè?c$j(vñk?R;¡½9¼Ñ?ïÄ´8g‹¼?Kj?Ri'?ã-?`KH·)¦…?yÉZÛ¥y?zƒøv?ïºÆ>8A?r£­c	îv?]»]1áø?f*€È"Ï?{. *iu?lpuEíÄ?ï§C.Ì?b­(×ä|È?d:CŠ{¾ò?J¾
Ïà? £ƒé1D?_£ymZp—?ïÄ};¦/?kKhï7ÇÌ?W
G'/?MŒÍ|e;¿?wþ:
óc?fù[µ®.C?ïOÎ×ì?¢…'Zøøc?cL¿'9?rð‹#¥Bº?"¥d1òÓ?¡‹ñãŒY?ïV¹cþ?¸´àœ‹Z?nÙ¤¡2‰?v2¢ÕLŒ?"¥K?t™ëÆÅ?ï&ñÓ¹È[?~i¥­pˆv?wôª¦x"?eº˜lq?•$šád«É?zKóÒjÞAGN4FGL J0125.4+3200?éB{‹DIåÀ>O…r›(À:o€Ãþ¬À<\\3Ý}@륹¸rù@­"BJ'k?ö9¿‹P?ˆ?ºPVڂB@ÒL(!²,?ï½ö=	¿êÊáÛQÊοìNß+t"¿Ú%|ª¤¿é<¢¨6¿ïøHEéïAGNbcuMG3 J012541+3152?ïâ3ô¤,E?lÊáÞnJ?LMdÈ':?IƔ`T?f¸±ÿ˜YY?j	}K•Ä?ïÛBVšI ?qõ¢,óë??·©dÐdC?Ikuý,Åí?pcZ)®…}?paå^Ò;?îÁô!ƒ?—ªÍ|?f¨Ü{Ɣ?r´éVR?¢v<}vÝ´?–A÷´;?ïñ†Ò¹î?C[3|Œ?@‹ç6ù3?-ž";Éø7?T¬gw•8?@,ÿÌÛ8Á?ïÊ,SÅúÌ?w†|fnþ?cÿû"1¿?d*•æ=Ú?pêG)=\?r'5Dw?ïŽpÂ(ü?ÖmP~
?YÊPO\Œ?tuà]Ç?‰A¥},Åi?‹`á¼ÿíd?íÐåÿ´çº?¢Îý»?o`]'÷ Û?uþ? ?°}ͯÐç?¡¦¿ìÆe ?ïÔdÆ«ä?c¥Ú¦ôZä?`E§xÍ?Y ÿ-	?kU'ð9cÑ?[ZJñâÑAGN4FGL J0125.7-0015¿ïÿú‹™H2ÀNó¼ÓZ…ˆÀ:>¨*VàÀ<eŒÿWc"@ôÀÙú\Ó@T‹<߄_?ÀÆÀCQŽh?µOm¦v¡È?îʾ­	c?ü©NM?ùÀ¿ÎÈ^éooÏ¿êY9W:¿éµO!ü)1¿ìn•	 º¿ïþôœõn­¿ïÊO[–AGNfsrqPKS 0122-005?ﰄ$ò?…–øY·d,?gOk"çÏE?elaÊ
?|D>æ0?'Hà2X?îÑû,S—?ªîøUB¥ã?‰¬—´M`?–Ië];?™:Ä2Z¬Z?¢ÍsV]Ÿ?ít÷Êb o? vzɉq9?"%/‹õi?uøxû›?¯땓9S?›c~L¯T?îï:éòÖ?Cnɝ&œ?&Ôý‰2b?veáz"¢ê?"…8IÙ¤?u™5ëO;ù?ïŸg':Z?'Ø
w~½þ?tè´¡í,?tÈfPãèˆ?{c'ý'Ð?zïÃê‹H?í 'b©˜?¼"Îó(è=?šr·\›?«	Ðî'p?°b¾–Õ?µþc¡'¿î?ìàŽØ†¦?¡4+RTÅ?"ì3܏}?ŽìYd]=A?´&—æ³u?ž+ý95³?ìÇ£þ¢]?¢A Vê?§¬†Xº¥Z?˜þçi?»€?«ã/h7×?•­—*—µAGN4FGL J0126.0-2221?É&_<rïXÀT3 ù	kºÀ9ú¤û¨'À<^–ªÑÐB@
'èý/@Qè´k­?¸çý)áÐÀ?¼Íé'e"@Tá@ùòìòB?ïdcâ}Ž ¿åÄ ]Øù+¿æ58%á;¿ìŸõÔ-¿á:ҙ•gÜ¿ïý› Ø<ÂAGNfsrq3FGL J0126.1-2227PKS 0123-226?ïúlü
Zª?@³³#‡?Iê*pp?ÉÊÒ2P?C'ï3ŠŸ?>C¸o%Z`?ïêÿLsB?iÕ¥¶ä?,ˆ3%¼ý?;DŽ<?c?
Çü"ç?gvý.év?ï´¶%Éñ¯?q9¬Ñh?U±ñG=?T؅ã—ä?€TNªÀ°?p	ejL(ê?ïô¸ì­õ?9óK¾¸P:?$§Š®5îÅ?OI¿{"?Sù6å%Ó^?9Å.‰¼E?ïõ~rTcã?I£,î].Ç?!«™nš@l?mš&CÕ?RͨO8z?H6´ù8â'?ïƝïGS¯?"¨Éë«??·œáïÈÔ?R,ƒ±í?zµŽ¨àð?€‡ïI%?ïv°ÿ€˜?'XÜÁà«?d"áxðʊ?hۈY±ÉP?W›Xœµi?€JxÈu*?ï݆™óÂÁ?\Ã1›î‰?@†Éðeäy?3³¢©$C?nW³À>Mˆ?[£kN×AGN4FGL J0126.5-1553¿ì³Æ̶//ÀSæ¯ÌâÀ;-Ù8ëÙØÀ<™Zž²O@9`<*Ô?ÿþøþƒÿ?ß±‰ÚÀ?ã=:ZMS?þ'PÀô*?þÝAאË¿ï•'¾´V?ã"; g~"¿å"]9–û¿é(ª^û'¿ïý}Ú rf¿ÑÓTÛúg:AGNbcuWISEA J012708.49-155554.1?ïXü.uo?ˆâX•¼l?mþ·Ùà+…?d0;)G\@?' £0¹¸?†õx|8kÊ?ï*øҗō?™¼Ÿsœ[ ?€mxZXé?ƒlÑÌ1?'j)xü'?'-,I¹C?í)oÃzn?¡ýü´.G?˜ÑÃ+¹AU?'ŠÃµC?°€¸Â?œéIøë?íóndzÞ>?ŽùÄÐc?†^§ÔeŠƒ?s"·
xhï?«1i‹]6?Œ"éâóö?î]ô]=%ƒ?¢Ï[©fCÀ?|嚙¶ÚN?tNá<­ô²?¦"ÖÑ
?¡ä<øP?î§¶ÆY?°^ÞÚ>Ë?'y…3"o«?ŸgLÑ{?¦òrí–š?¦ ®ý'4W?뽉xí°%?§kh	ÒÝ?ž…¿þûK¥?'dôŒ´wÏ?ºrD;ÕTl?¤PìHìl ?ëÙ%íò¯?¥Ò5.šy?ŠìRÞ{O?†›˜!tnè?ÀÖ:Îvà?¥« ÀAGN4FGL J0127.1+3310?ì~§!ŽèÀ=~À¨À;MPïܹÀ<±­ÂEŠN@ wzÜÀ	ñ?ÿ:ŠÅÁ?Ñ?Ë)¬ ÚÁ?šúv~6'·?Ó°È_TÏ:?þù$f'¯j¿î̞ßS¸?ï—L¸?w¿ãþÊuÚx¿äWewS´¿Á¢@Ýîz¿âÛea-Â[AGNbllNVSS J012656+330727?ïÏÙÂ(®ö?oŠkö=Ÿv?9c"žá*î?+£˜š?v|å§æì?n™ûÞ1?ïÈcي˜?{67žÎžö?F•Ìëõ#m?S'W5:U?xûƒõ¤Ò?x›QÂüÓ?ïZ†­8?|øÃ`Àq¹?`UŒÚ²~C?VgÓLèkÝ?'¤Œ,lÇ3?z۔iB´'?ï™Q‹@™?gƒøKll:?O¾ßùñZ…?=laÜú¦?‡¯¯9üÁ€?gyž¸£†?ï"õuk?€°‡Ã•'ê?JÍÿªØÒ?@¯2©xV?‰'"™áQº?€38œ=µ±?ïKö!4¬?•ècWóo?[Z‹2åë?pn}ëJÐ?"Ë"1¦"?"(êÆ7%i?îÎÂ~â?‰CŒÚ‰ó?ftöL[?dqÄ?¡¸r³â×6?ˆ'kïV(o?îå|—¼Zö?†qAâô~?`mÇkãÎ?X~¶<:Ä? ¡dÖM¼è?†HN?¬|ñAGN4FGL J0127.2-0819¿×¸œ­äîñÀQXh‡¨ÖMÀ9…(šRýÀ<>EJŒì@°áõ(
¶@ÒD}ÞR0?²¦¶¸ŽQg?¹	ÜÞÎé@ìÜ¢,æ@¦+
DÒm?ïÿá—_,¶¿à2f9Œê¿â?™s,Û¿ã­_I;³¿äÀÉë£R¿ïüäÝdʅAGNbll3FGL J0127.1-0818PMN J0127-0821?ïŒmݺA?€³Í@	?POQÉËF?Dª±¶­?ŠÚžO>Š2?~ËT"QC¬?îYz×ÙèŒ?´…m]h Y?"ñWk'Í?£ñz}ß? ÛYÓ<å?­v
vã?î	¹$¬æ0?)¦ƒ'k?z<NÅ?Iò±E¯M?§'c—æ!n?—«PU¹?íÕôEâS?‡/´0?–7'/ËqC?x
æí¦‰?§"ó<õ"?2Ôê+Æ?ƒu§?K{ȶ?k^Ø"Ôá?dmQEy¨)?¤¦Ù?™??›á‹±ÏI?ì÷'üô1ì?½ß6åLþê?¡þ#
_ï?±Qv'LÒÀ?®]'8Ù.?±à¼8*ù?ìP«›¯I?¥èʘ	ä•?É@#u?–I›î]–?¶4°á´»^?£V¥"?Ä1?êÿßq<X?¡W#"OþI?©ŸF:x¬!?ón€¹	?»1d]ïì¯?šm¯ìþVÄAGN4FGL J0127.2+0324¿ÔŽ=5ü¢dÀM ÖÓõ¶À9ëRV)ŽÀ<A¬½ã%@ª—mÅU?þƒ=¢!þX?¸–_×Öì?©"U´?òŸ£ž\w@XS­&>X¿å¶À'¢Ü¿ÁfA''–¿á,Xï
¿Ø͙ÞA¿Þ"â¨V¿âôN>aAGNbll3FGL J0127.2+0325NVSS J012713+032259?ïûu^HW)?.Ïþó»g{?w^&ŸÛi?dvô5l·??÷5 ¾[?,{qÆP?ïòRN—?bsËòŽÕª?&u&Y¾€?89~bT:?Y ¶s
û?`yq+;Ž?ïË"'ƒIî?[ÆËYá?MòŠr_á[?5Åꈪ@L?v°muGn?Xa©íÞ´?ïíu÷Jq??d¾eþ^"?‹`s˜¶?	g᪠Ú?b0/ø?>˜‹°¥­z?ïùޚC|p?4''?gò?ŸF¢Ú?
:¬Ù¾?DÑ´¨2ð®?26ô©¾ ñ?ïÔS&B´Û?}ÿß»;PË?9³©Æ€ý?P"ѾWÞ?t;;{:bÄ?{»£ê¶XË?ï®IÃ1\?maµzìGv?XCþ6À?až¨þ£e?sKxº¬?eñÛGän?ïÓÒßò€?\'@̹Û?,…Ç™i~?_û€.2?uŒèR± ?[Õæé	eAGN4FGL J0127.4-4813¿à:ò†^˜+ÀPñ(Œç°À:¡îàªÀ<±HÒé4@6\>šD@¬u>p~?½¬Žé½Hu¿›íµ^\µ?ÝxÞ8/v@[–ˆB.?Š&Ã‰à¿ééŸ"w¿å¶?A´U¿á¤•á~4¹¿ïÿü¥¬¨?ïÿÍ
	n>AGNbcuPMN J0127-4813?ïê@dâñ?n¦°hž*?L`_Å^?D8«ýë?]v±|U6K?mó8k1Iu?ï×¹2ø6?s5(¹Ü'?AÝPcm?L¤ym‰¦?qçÆgÜÄ?pÊ?f¸¿Ñ?ˆ)"´?|sÃÀe
?bÃuv&àX?lv"´Éj?ƒlÀnQ
?xIly0³ž?ïé÷e°;¥?I=J"– F?<·{Õf?&—<ÐÁ ?bqª''Jº?F²+‰—?ïÆ4eÉn°?tdr¡*X(?dJ£ßèX?_,ÖrG)?rÀ{&–ž?pö^ùƒÕ?ï=ÈÍ?Œ}˜¢œÏ8?UtBd®÷>?aH{ô2?Š¨9{"ù?ŠviÏ@?ïS"b‡!?…ž%",p?hdrÎ{?oàÍ´û2?''ò4ў?ƒ‰HX{?ï³íí½??nn©"#>7?Yr{³'¶m?LˆG]×g?¬jg4$?kކÄc÷hAGN4FGL J0127.9+4857¿î×µþ¡}‹À*÷´ÜëÿÀ:9ƒ^ıuÀ<%'¡}"@ãþàEP@؝jßqë?½"¿Àéz¿*ò¿Gœ?Û÷ƒÈL
@v¢ÔUØ$¿Å/"Â͚}¿å"wvY"±¿ãNU}àÖo¿ê\ \–ÙÌ¿ëEMýcîg?ÖºqëÕ¦AGNbll3FGL J0127.6+4851GB6 J0128+4901?ïßÈQ?c8¶§ß?Ez"¤#o?8ËètpŽ"?jÙ\C??a~ãîyU?ïÎhËÆgƒ?xžä¿?GK/²â
?RºIF'?uâ9¸¶Ôä?veóÏnx?c¨_Ê?Lè¸|
?fêùúž?n°˜E%?‡Ÿdè?¢‹?}'w¥IÄN?ï´ÊúSˆ?^gRªˆÞm?PÞ ³¹h?5à¡ÂÎ?€ãyGƒ?\0ÐÄ?ïj½™[¹Ã?©G:6
¬?t""3R?¨ðÉ^áÀW?‹?WšðC?…CÛÜf3?ïoÕh&Úà?"g"žÇs?^P$
™\˜?q¾°Ò? P¼âÈ,?'QÔ{?ïšËëæ?Ž+BJ"§0?wo×m('3?z -Ãð͸?™°©åóä?ˆµ—Ì\Ø?ïáÛÒ¤'?rADO±Š?jýur±?XÕâXýؕ?›¤Òó~?€Sú0¸AGN4FGL J0128.2+4400¿Ý/®|]QGÀ2^ê šª;À:ñJ¤iuÀ<gÕÈc@}"‹›)@2mæÎ?ÒÓJàxü?Þv­*@pZ:Þù@'N¤RÛ?ïùHUÚ'(¿â£«€ÌÄ¿é	¬AU¿å
" ®¡>¿ïÿ÷fÔJp?ï¢O¥YÁAGNbcuMG4 J012818+4405?ï&J¿ÁÌi?˜0áý¿ª?~ŽÆ¢&^ ?"ç b¶ƒŠ?"'öe˜"[?':ñ8T?îíˆâšÇö?£ü÷×}Û?†µŒYK=?'–Ù…HÒø?–ôXaRñ¹?žvéÔ5?î:ÓÀSd#?™,ÝèÐz?¦‡ÓCj€?ˆ¤yô&~?£ÿ€»½"?"3G"¹ìè?íáðÉ3î£?Œk¿P>Z#?'}‡oi}?u9Ž¥ut?¨¢/±œ»O?‡	z8fŠ	?îXi˜Êçš?¨©8¾¥|?‹#€	f
j?Š¶`ÔËÁ?£°†l¬€Æ?¦N¸ƒkd:?ì¥OÝÛ?½Þ'=?§ˆXƒÃ§?±¿h(&?³Ç"ÃdðÐ?·ÛïQøi_?ìsŠÅÛã?¤øхÀµ?œ«vý­	?'õ–ùów?µ8Ì-H&?¡½Ü°IÓA?è{säÜÁ•?¨à"&Ð*N?¬ÝŒ¬ƒþ"?–¹	Hš0?ÆÚÍ@?¥âRÅõ˜AGN4FGL J0128.3+5710¿äºôœŽZeÀ^ÒàD²À:…	ËZÝÀ;ö÷ÛnP@@Ê?SÒæ@f–DzƒT?ÀË0šÁ¸¿¨tæ†Ý)f?æÊÐê°
@6hk#d‰?ä?}ïD¿á©ýýÇA¿éÖ.u^Q¿çÀÔÁÔi¿ÄÚWåD<ñ¿äMHˆ/AGNbcu2MASS J01282987+5712494?ïEÜP«ò•?ŽNU¶•?aZ·†Ë?Tôc'=.?•5oÉG¤?HcaV?èK¤',N#?¾ZÅæÌ?lªÇŽ|^?vûêöô3?Î^˜–d[?½"²tåbÎ?íÎ&ÒZ]ø?šÒ]Ε¹?uQÙ_»î?qn¯Ææ´?°9«Û+-'?šÄ7³8?ï<P‡p»ï?spáxX;ã?Hi×úëuÕ?4F×Y*ö?—² YYì
?s3ïë½­:?î¾±ùY??¥šOç'Ù‰?w{¤(ýCõ?oøW¡ÈÙJ?¬T ^biŠ?¤…‡#ê#?áç;JPR ?ÆÑýŒöÌ?kubŠ‹û?~—Ã
k;?Ûúž§J‡8?Ɨ‹³Ž¡?êì8Šò?ªŽ£T*?"ÂSɗu?| (
'?Ãœ¾MiQ?©:ò<š{q?íBY–Ê1g?"®RGÒOä?fÞ$Ê j?\ §yYôÅ?µ6B#&zÝ?"RJž¶nOAGN4FGL J0128.5+4440¿à&nSÅ¥À1±Û˜AªÅÀ;"|úÀ<ŸÍHÏD@'³Jß@£a™x?τ"ú£tº?ÒÁqºWC@÷~0‡‡@
^~\&q"¿ïÿ	ËZÜÅ?ïþ¹ä'¼0¿à~ø=¾Òc¿àéÔå i¿âËNÀŸm¿ïýjŽê/AGNfsrq3FGL J0128.5+4430GB6 J0128+4439?ïõaÚ¡²Ô?F'^N`Ù?3ÖÜC+ª?( a_eÁH?PF"Ï‹‡?B»ê7s,h?ïÖý¸Û†×?r‡h1·?E›úØ&'?R±²xØÃ?qͤQó+ ?p2­$Y‡K?ïv	³2?…ù"ù"úû?mÏ-IÄ* ?uÓ8ƒJì?‹°á+Jÿ?'`˜¨F×?ï‡X¯¢"2?fu¯É?d¼öLY?En.t´ˆ?ˆú–• i+?d͞!2N?ïíQiÕÖ?S|Ë&2Zw?D%4í¶ØW?96\Œõ5L?[J'd:?O"y°8¼€?ï|íHdÀ?''?Ïy?c«%÷ˆ?uäu¶?‹Ùè^æ¤Á?! i¹?ï;@@ó÷D?ŠàR""÷4?oŸy–®¦?tÏ6ì?"¤½¦¯¦?‡K¯=úõ?î¾:1múô?ƒä˜'%æ?vŸ–Ê»‡K?aå:«]y?¡HjºÄT?'ï'ŸfyAGN4FGL J0129.0+6312?³wO8?äÇ|Ìy1À9VÚÎO¨À;(Âñ·ü@)Ûp©‹@‰‰>ÃO?ŸIO@?ÑÏᗊ @"ßBñX?þ[^¸ù?ê|Iâ¢!(¿ÜJÐÞªDã¿è+b€=¿èr(;ˆl¿ïþSÝͦ?B§D}AGNbcu3FGL J0128.4+62572MASS J01283059+6306298?ÛùT&•7'?Ä*óxÞ?¼äƒD:?°µy¨¿?Ü͋\Dú?ÃIÆ:¿ø?ÔS–Náe?ÍN¼jmÌ?ºü2.ë?²&)$/—ð?â"ÒõRIp?̠Ս¡Î?Ý$¥'I"ó?²^Sú&m?½DŒt?¢gEDµ?ۊ7h™hê?±Û³¡Ãä»?ØTƒÑÇ]?«ÝEs…;?ƞµÌD?¡§¥r,?Ü\|%H£?©¨dpiŠã?Ä{ãבˆ?¶i׬;?Áä¨Xh?·3Œ¨Ó?ægÝ"Çâ?Áué6öóM?»ã0ðt?Àð˜®ã?Áp+gž?¾QÂʞ?è''¿pÿÙ?Æ*.®$|G?Í¢ý!©¢?¯VÿÙÌY?Àñ²ü'i?¨»æˆ{2R?äZÓø²{4?³ì"Ì?¿êóÜä¦?ŸÏmAö?Ñ°±Ž$h?±|§cO?ãGȽQ7?²+""·:MIXED4FGL J0129.7+3436?ïÈ}?çÀ;—{Zê1bÀ:ΪcyÀ<¢|(oŠÒ@©…©	¤?üYo!öÊÍ?Ì2T¦uu"?ÑèßZ©š@ÂE¿ý±q?ü;ÓÐÍŽ¿í^¨âŒÒŒ?ïÿŠ#ÚМ¿à?(¿'ÐͿێÅ?º«¿ã;½pcj¿ïþ2Ö!ªAGNbcuTXS 0126+343?ïâÎù¼U?by"ӝL0?Eˆ\"4?Ay'`;úO?gÎïÈ"'?_ë$gǜ?ï rcG7?– ©—äCÔ?~²ú,­»?"š£.?"E2d+M·?"7|Yr?ïü~b¨ä?/ºn*žó?~ZšïDÈ?€ðrِNr?˜™"¢OD?Š4ê&Ì^?íÀ˜x©¬?"+—²]¢?˜f·/†ÊB?u"y¥£Š)?§ÌšßÖ?€‰$?¸ò?ïÂGsd¯5?q%Û¢ùA?]Fs!úÂ?TÓ«>ÙÄ?w–tÌ\ÆÊ?l™î¾c!h?í3‡åÎ6À?°ÿ¥­ÍN?™*D)Ù ?¤ Oàâ_?°"6@à5?¥@¿!ŽQ.?îŒÅ¿Ë?•Rà'iŽ(?…+"óW@¨?"ÿŒ˜›?¡èÍÃɗ.?'²²Êa?ël\ùÖ?š.¡ÒBðz?¤kûѝ&?MIÕÏ?ºio/bÄ?•ñd¢:(ÐAGN4FGL J0129.8+1440?…•ªÊå4ÀG"ÇŽŸj"À9ü¹w…r›À<UÍ&Žà@‹]†6@ø6Ã
¬+?¼÷¾=?Ňz]>J@8âe+Ô@uÏm À?áÛނ׶5¿äÄÏ"¢À¿ëSÕ£Ï(¿æü":µ´¿ïÿØ'sâP?ïýgr0õAGNfsrq3FGL J0130.8+14414C +14.06?ï;ìD-ν?µÔZ¢ZTØ?Š²·§ëy³?¦žwA-†q?†R7EÁŸ*?§
4‹rÆc?ïN«ÇÞs?"z,؇2?vŒ‰S6ñ÷?€Ú®R\oø?‡yïJÊ*?‰˜2*8|?ï4bÝÈë?‹±Tb	K?v2ù4qµ?va2Š—Ï9?"ææ†./?ˆ¼VHf?2?ï£õӁFç?fÉmØܶ¶?pî°ÅUÅ9?X'¢cՂø?}e›á?_±¢]c7?ï3>©"?–½vWET?'㏀?'™}åÀ?€<âŽGz?}šÜ׈Dä?î3ÏA`r?«qöæœnÆ?ˆà4¡‰?—ó£·³>?¦Šþå"?¤×8-z?î0éŸôÛ?šŠ›'wãó?'C…ô¿°?Š[hØòÐ?¤O£y"Ö?"|¶_ɸ?îŶðŽë7?‰›g؉÷ï?ŽÖ"ô.À§?"Mÿ}©B?—Ý×t8Å?€koel¯AGN4FGL J0130.4-2129?ì7á.:{ÀSޞ²gÇÀ;8Ov_ÙÀ<Äå°Éa@ 90ƒUŠv?þK¡ô±î$?Ê,ëš?®.‹qYM?à…{ÕctD@xUy"%i¿ïø•½ìà?ïÿèþ†®/¿æ/:€.¿Ó+u¤œ×è¿àqÏP4˺¿â•=×AGNbcu2MASS J01302573-2128389?ïñyÚ.¼?c7ç
oô?*x
g?.­Hœúãá?Y½K˜	lª?a'ã?ŽN?ïàÎr1?oÿBç?;þ½JE,?Eí$²nú?k²* Oß?lEˆܲÀ?}@?wڂ?ÿU?`i{°VÊ¿?g1´ÃG?Š!þÂ
7=?sŸ¶ÑOH×?ï¼×=áYn?^
‡¡¬.
?K±¼Â¸È?3¤à&}m?~)€å`?]@Uîd›7?ïë{{©ø?YGÈ?A,õ?:ýqQÉBÌ?:ƒZ4A?aÖtéÓm?VJ»g±'?Arø+?Š'Ž?N)œ´ù=?]y¾ãû–?…2•Ðø…¬?ˆSÃYX!Y?ïEkªv?WÓ`½¢?cq-à¨Ó?g?u›–~œ?"äeŠ°?0º	2"!?ï`—ß!î?xý4>+•?[ØD6}ÿ?OÞ)•¬?'/Öl6I?xc;
(­AGN4FGL J0130.6+1844¿êJõ¶ó>ÀE"C•%À:·t×Bq•À<zd׍@D§ú°`@؞wNëö?½£‰¤^¦Š<¿f?çm°r#3?ûÒÖ+›9W?ëÙßYí1¿ã¼§ñK1W¿èy6ýîü¿Ùö?¿æËxÚq3¿äã߸âµAGNbcuMG1 J013030+1843?ïÁôU6?»‡IȊ?DÀÕj¹®?5ø®ó²¡?|mÝ¢ª?¹¾a«êË?ï€ÙÖíÚ[?†ë³Ò0ã?d׬ŠD5?aaT։u?ŠÆT`õü+?"¾¼[
Å?ïo¥n'êš?w€yêÃ?gÉ%/‡Õ"?gR£tŽþ?Ž$[5"$,?sAG4ÕDJ?îáìÝʇ3?x"mãfþ?yÎjá¿/þ?Z²Dì‡<÷?Nɉã™?vƒyËÉÕ?ïƒF:Ð?ƒº/'ô÷ª?]7Á‡$D)?O±U›jO?‹‡†;j?'³GFæÆU?îÄê©	VÉ?œŽåx¤³Q?qmS½g?stó63éË?¡§ÁEGA?šq2-Šä?ïa¦ì›þ?"6¯5­vô?séWF¿?oó›ADB?šnËL–?'9—`Mð?ìv‹U;Ï?"–Î6yü«?"Î:A6¯~?1
~|q?¶P½,Ž¨?"Ù¦^æ`AGN4FGL J0131.1+6120¿ÛƒŽÇ"»¿ò¯bXº¬9À8Ê&LšãFÀ;™Ô	×ð@ œxfn?ú'ƁY0ô?«_§/"R
?´dsá½äk@mgŸKŠB@5êhi ¿ïìk˜ÕN|?ï5O؅g³¿ÒÑ@"ªt2¿Õ¼`Ï"½¿Ú\"»;*¿×fq#-×AGNbll3FGL J0131.2+6120RX J0131.0+6120?ï´µ9]—?†;­ÔYÌ	?9'þ5¾¥?;p»˜"…C?'	xÐO{ý?…ñHXéŽ?ê'SFE?Ê~`ð¨«?_»<ed1?tª·vÀÐç?Å·<lÂËí?ÊNbÓM´-?î´UÌT?›òóÖe¢¨?wô¿¿"<?j4¹?¬v"«'x‹?šÁ|?II©?ïAòSMã?qÍ+h¢Ïx?_¹€ñME?@óéšÉïå?•Æ&ŒÔÉ?pòÒ§œ?îß~ꅉ0? õc5WÆS?QN™qOÖ\?S½§µ?¡}œ‹WË? "$'q‡?揃êì?ύ©IBœ»?sYœùÕTj?–  Ô3cÿ?Ҕbƒéë'?ÏœÂ_?ì¾ýŠk¨?¤ËÀ. °?€Ýbݝ?"×°Ó~˜?·ìgOæ	n?£ý­à+,?îr•Rs"?‹–<íÇX?o+!hæÖ?Xë;iK=?¦ãýwÜÒÌ?ŠÕ!Úñ'ËAGN4FGL J0131.2+5547¿îúÓÎÒ>.À›œÆtÄÀ9Ѳ–À¡EÀ<Úìô‹@	²:zOQ@Ç>'Ä?¶)G!&Á5?' Cò7?ÚÉmÝ(9°?ðìÌKós€?ëÓåjR"¿ÒD¬{*C¿ä"éœl_¿á¢>ƒÉM¼¿áèi«•D ¿á?áíEhAGNbcu3FGL J0131.3+5548TXS 0128+554?ì¨1É?"?®UÚFðÅÉ?y'TÁÀڜ?mÎîSÒ?¹'	&–Øú?­xs°,X?Ↄ‡W?ÈrLE?Y8…¡wÜ?ŒÇKàQ"š?Ùø/-·j²?ÂÌMǚD ?퀪ñõj?œN@EcŽ$?"­bnøÖ?~™y@8?±dü$-zÅ?™ç"ö²ÿe?陏Rîº]?Ÿ‹'ùJ?­tÇ҄J?ŒˆëŒÛ?Â<ºÂ{¸?–²ˆ
ÍyË?èßgy`éû?µÜ&=‹¹£?Œ)þJ+ô?€i`i­	?Ê¿Â5¢¬Æ?µvóÔoû³?Ñ,at†‡?ÂáZ8Ô%?–'Óèü¬"? "ª§¼z£?渐¦g¤?Ã;‹W±è?ê¡,ÄóÔ<?¦JòŽõž?'ê_MÑÈ?ƒ7Zƒý)?Ã>.ZS?¥`q*¾?âK¡Åü½Å?¯L{»"V?¿ÓÃ#Õ%? Õ¥Ý,"?Ós˔=-?«p'2ņ$MIXED4FGL J0132.7-1654?™`ñPÀS0#̎À8qŽ©{ŽíÀ;âêJŒM@»ãr€¦@&ÝA‰?œS蛛¡?¯" î@UL}‡\@:T‡–·½?¨­[ î*H¿âgwÞ]îÉ¿å"Â<Pg¿åfÿš6¿æ-À×K+¿ïÿƒ}ùUAGNfsrq3FGL J0132.6-1655PKS 0130-17?ïïý÷ŧr?Qër¡R‹–?8vÃF?/'nHò0?Z2•3šk?P+Õ¿%¼æ?ïåíu‡c?o'k—ȝ	?5Þgq=h~?J/]AÆ}?gW,zÇóO?l0^<*c?ïœÏ2å[?à½ð½ú?bŽGr,²®?n¤"	Oê?"(­^J §?æûü€
À?ïö$œË?5Wlïz£?'Œ–á1ó?œQJ´îF?PÜ$=×èé?2æü…Rœ?ïÙ-'N:?iA\]M^ë?BÅr¨ó°³?7¶ˆØßÄÏ?qˆb~Î?gêælsÚ7?ïÄ0.y˜¦?'XW1®?GÁºN¿ŽO?a‰4än?zï±l¶Äó?€lø$Œ?ïHµÂò?M <Ž
?fÇ^u?p¾=–M/?"`(t¥?Ž¼úþ«š?ï뒼Ÿqå?Q@Iùõ?8ˆp"'?.ø	(fÅÓ?a[2šuÑW?Nþ'	nƒAGN4FGL J0132.7-0804?ÖÆànÄÀQ%EŒÒ
úÀ:½%eëdÀ<{Y"M@ >_W(…Û?ü4sT‹r?ÆlN'^?ÂÌP{£`?ý9ƒ)Ì@?ûdÚ­‹¿ïÿù&Çë?ïüe@Ìxê¿«{ŒDg}¿ß,ÐÃ|l¿âªo¥Ó¿ßæ‹d͊AGNbcu3FGL J0132.5-0802PKS 0130-083?ïÏ_áçç?fIí´ÎÔ9??º
µÉëß?1ý:§ÒG?vTn.Ä_?eRáP?ï³SœÉv?'ß{jú]Ë?]µv^t?gD»ýÑ?"ÂÿçÕ?~Á±hH]?ïpnQŽµ\?€cÚþÝL?aq Øï?bæÁKT‰:?ˆ#™oú¥?)Y>?î"i»c!?ƒè=4I¤?+£¥iº?a¯ÀöÅ?©ð´ò0K²?'XiÍrêÑ?ࡖ?wª/I´Ëï?W…"Óƒï'?N™ú‰;Ý
?"aG/Î֑?v'ˆK9?ï)†´ît?ž~¹6y?p²7Et§ê?}yóãDd?–¢›¬Ê"?›bÿn¡?ï0Xð²J?":†Zî4?fÓUñÜÎ8?`z`µÌ¦ô?—w+ƒÝ?'šŸ†8¢?ì8à®3¸?š‡*Ü@•ï?ˆdèðý1?v¢ˆiê)'?»3[üC÷•?™ÂòN(¼iAGN4FGL J0132.8-4413¿ïòÇhúÀQ¿!>>)0À:W]$žDúÀ<¬wD@œÒá¹ÃÜ@"¡ã6ï?³"jŽSš¿«¾Ùo˜g?÷ûƒ™}?üSÙÆÛF¿ÕéC¥ò¿ç5ø¿ßHƒ|vÉ
¿ãÒ. ý;*¿è›_Óû?Ðؗ;ˆBAGNbll3FGL J0133.0-4413SUMSS J013306-441422?íÀ/Ž°T?½*0ïÐÍ?z—‰lÐ`Ê?•KD?†9?°UÕî‹BÒ?ºÞ>(š4?'&?…:»G&J¼?b¼¼Nœe'?gó2oä?'Ï
%3?€Ü€fEC?íþ3«9ec? ArPªgr?†'	­sƒ??ˆk`ŽD­­?ª"ݝ-?'k_ºôµ?ïZiR©ñ?thèlՇ,?sLmå‹]Š?^ý "‰‰1?¿tR?ñe?q_ëBà?ëŸb4ÂCK?À‰6
òË©?ßÔpÂü8?'ïz¼£?¿HóÊùŸ$?¿ñ]rCa?îöA\¹
ð?£ L•s³ñ?x¡ªÆMèÒ?‹vq˜Àù?›i½Nx¶?ŸFœò1›?í¡R0á?£ÿV8¦!®?WiÝå?Ž®5]?³‰P~Ñõ?¢A—\Ïû?íþF‰ýq?"ÇÀîø:?³_ºï?Û±cß&W?¨®Ó‰Ëw?'e©_‰OAGN4FGL J0132.8+4324?Þnr4¶ýÀ2ÔUGZ2À:œ½‡µk‡À<~ÝW^‹§@Ÿ™¯i·@|¦ˆÃ?Å覺YX?ÏèªäD¸—@*%£'·Õ@Q»úA¥¿êN›n…ð?×ò)é•ö¿æÜ¢˜E܃¿è6'@Œ¿ç¯§"X¼¿Ò6ÓfD¸AGNbcu3FGL J0133.3+4324B3 0129+431?女ۦž)?tEîU©C?WX7uÌX³?KArÆ°ûÎ?ƒt'жÑ?r맶ñKæ?ï˜Ó#[­X?…üy2§å:?fÂ! Ù¸Ç?t riíù?"®à†E²?÷¨ŸF?ï#×W5Ù?†‡xÚ²=ª?w¾òuÔª?sêÈqv?••Xz)x?'nè&­±Y?ï?+
—9º?m<M¾BÔ
?€V»U]ü?[Qªº·?ÞÚó_?ixȽ˜WG?î÷¯ęÖ?'Fç¤S?s*ZFsC?m,Gr¹'ª?œ?…—}6l?ŽÿAܲü?'wWê?¨.7¸ó?‰­aBRDw?Ÿ²ü÷Ié|?žÒ	¨Œ?«XÛNÊÝ?î4èi'Çè?•ôc¿G?Œn4ž¿´'?†Ôéð¬Íi?¥•ì=ßZ?†vH©š?íÂ×õŽ¦»?f?¡–î8?—akZ
]?}U%ˆê¯?¨!Êù4  ?‰8\§p¨ÒAGN4FGL J0133.1-5201?æôþ>VIZÀOó'½RÀ8¸_b"À<Ûä—Ä­@a–8¼@ÐlÚ"?¡¹nÝ>›,?´ØœŽÁy]@}<y-ˆ@zdËÍ¿¸tsß²¿á%ĵ§Z¿åŒÙ݁zê¿äIê.Ýc¿ç-""aSØ¿ïÿGþò8íAGNfsrq3FGL J0133.2-5159PKS 0131-522?ïßuòܒ#?¡IdNiV?B¯cr¯i~?>¬Æua2'?kÞ4KJ5?¡L$룥Ø?ïñly"{?eCêøžB9?.
"§)H–?SV'›?Yf‡ÿ¬]Ã?^ˆGP8_?ïœh"3ÆM?ƒ†ÐFÝg­?d,¥Èw¶?q¿ü뇧Ç?ƒÚ±½Øã8?'ž8Ž^¡?ïþ—f¨Dq?¼¯Xç_>ð°ešÖ"@>ârôk4Z?$s‰ÆËkë?ˆB[4'1?ï؅Ÿ‰3?höeº?Ion9ù?@j'"MLg?pB]´š^?f¶‰÷8à?ïÕæÇâï?|Æ_CÓ?AÒDW܈?bõ!ØRt?rÒS¼™§?xÛ:±&]?ïb·ÌÜ`?Œ7¼y™©?bÏ~Ûkî?n¤½eÛäÞ?'OÀ@4i?‹›Ïëw?ïüë@³×ç?,¶W_A?oywòú>ý',2?ö)?6X~*š"?*½}Àœ>AGN4FGL J0133.2-4533?˖Bï`BÀQrŸ˜·À;·.Hè§À<ÿ'zç&ë@!Í\áb0?ìišÎM?å‹ÿ'=?åÓ°ìœuí?þëªX-¾?ò'.䬿ÙäŨ¹?í,{ž†é>¿í¤.}ÁÌ¿?ÒÄîý#VÇ¿Ö+ò¢xf¿Õ>ºÛˆ§YAGNbcu1RXS J013308.8-453528?§…Œê?³
ÀNÐwÆ?}o½ƒªÙ+?¬uM1]±?¢·MÖöÂ?¨Ð·ã½œ\?v"­:?ŽŠ}§2¤ç?iE|â*äO?{Ð@	†l»?ƒ<
H_?ƒÖ
"ïŸZ?í²3ª(Œ? íT½Ø¤X?‡IaÑ^ài?ˆc
Oû"+?¯
lé­ñ$?Ÿ3|äjç?í¨b§Xä?—íàx
H?s†=QÁý?p 1WH¸Â?±†ùÏ'?–Úd@ð€É?îJ\³î?¨ekÓXo<?ƒmw5V?…‡¥W;Eé?¦™îÚüB?¦JgòÌsˆ?îò÷*2Gj?§VåÊ1­p?x§õ·°'?‰4AŽ_è?›™ð½¨þ£?¤}Á—µJ?í`€Í‰¤ô?¢2gmbß?…o
Zê	Þ?ˆðŽ:C\?²NI1~&? ¡ñ,ؚ?ëg²
Ù²c?°2ß5D
?r´Ÿ¢þ¸N?|Î
x¯Ô?Á˒Ì1,¯?°ÿ%ÜÕÑAGN4FGL J0134.3-3842¿å˜PDw9"ÀR֜wškQÀ:í—û3èeÀ<ÆÝåùÄ}@åçØkç@n£f¡õ‰?ÅEp!¦?ºd]þ7ÿ?ñ oÇ88V@-âÃJb¿ÎY	†'¿ÖZ–d
0¿çD[C¢¿å[«!Z¿ïý¶¿oA+¿ïþë-
$FAGNfsrq3FGL J0134.3-3842PMN J0134-3843?ïð­'c´?ƒ~‹B>l?9XcÆ£\?Wv螠MÃ?Y˜ xm"n?€Ò?Jì)?ïâ	
߀r?pÃGŒ_`?:Î¥ÆtØ=?J鳊}Ç?jPSš©?lÿ›Éak?ï£çIês–?=wãG?a9…ýàª?ip/äYfe?'·Ì*ª"d?R;Š[?ïåÒÚOc¸?H¢[|g"?C¨þZ·•¡?)›¾8Ñ9¡?eBæRœ?FJCDt5s?ïÚt#Ø<?žÎ_ë?R´çI™Ø?€r¾˜ƒ'?l1h'A‰Ù?–Ÿ½jŽ|?遼Ú^c?ˆÈŒ6´»í?Q2©ôþ=·?aý†ÎoÊø?ƒøÊÑOáe?†U×R*Òä?ïtC§—?‡»>5îð?aÿ%E'?kñå´•?Ž{s[Ýj?†FBM(B?ﶒÿ/>?j¤<N© ?Yê{òßB?H<J¿w`?~;áXN8†?hTÖ<ÖSÃAGN4FGL J0134.5+2637¿î8B]¨ÀA oÞµ,À9U"¢ß"yÀ<
:䜸@@‰°îIõ?ÿ@7þtÆ?±:Çw"?šTg¥™H?ésñ~Ý֊@EZ¨6¿¸³ÿÌS€¿æÀ|ôGe¿ãÚpßf,…¿Ï‹Íþûô¿ã7a@6ÑοâV¢8¤Œ<AGNfsrq3FGL J0134.5+2638RX J0134.4+2638?ï¨ÑɍY?wéߓ¬?Sg†Øӕ?DDì"KzŸ?ƒ^ª+¡gC?v²»L?ï«K#P"h?‰þ±BЫ?UönƧ…?d¨Ž'ï$g?'nv£ðì?…žˆK%ˆÊ?îéd3Ê÷y?øƒu&?qç©ÉœÔ}?q)TSfžã?žYaE­?ú	Ž"?îÐÉÐ)^Ú?|{ã÷Cíb?uÅ2ČX1?YjQ_rœ? :¼¦zWÔ?yLñ¿Ý:'?ï|ƒO?'ìU9~
?lJäÀ'J?^ œUª7<?˜Ç"•‹ì?•Ãºï–?îé!C$K?ŸDAÎV¯?f%ϝ	¯7?q#º9W? ðÉCe?ÿRMX7?í¥H3û? šYÞÈÁ³?~'AA!¶?yÖ>]¯BÙ?°óJSÏú˜?Ÿåè¢wUû?í,@Â+ÍÓ?—˜A<Ò?‹®"H9E?vóBQé¶?³('e,| ?"ÍÙHMzAGN4FGL J0135.0+5338¿é¢V"ê»ÔÀ!^3‹GÇ?À;&ԅ'òÀ<´¯L¤@#hŸ§@Kj¿'zç?ԙ¨}b+n?æý6Œ"a@×'j@@ñ#
Ì?ïýÚ¡K¿œ¿Åz‡Á…Ç¿áû3¢™Èi¿ëß3םá'¿ïÿú÷''ý?ä™'¥RAGNbcuLQAC 023+053?Ýû˜¿K|M?È÷Sf·ù?ǪnçFÿ!?Ç[ŸÍ˜Ø?Ö//Í#?ÅÅMX»Í?ÝÓ_&ðÉp?ɑ,¼æ>¨?µ_(,å~Y?µÍEµÛˆ?ÜÔÖÍgãz?Ç\½ÈDtF?ä`Ò}»ÂŽ?²—Ø®'QE?€gE«Ó$?¨'X@{Â?ËüNÃe"¢?¬ö]A‰8?éc®ÛËk?£c±¾$?»üÈc®L?šù¥ú¤A*?¸åÀ¼,È^?—|Á¡¿e®?Õ £õh!?ÂÕXF¼†?ÅpÑ#s¢?À·ÆºRæq?à½äžòì?Æ|Jœdæ?͖Á‰3D?Çì'SÃæ?Ä	-XÜC?Ã
,ԟT?ãšMR]Þ?ÊhJ¹"?Û¼ô¬é¿?µvô8§)?΋˜,º§?°ý–ù/?Õ?F1<¸î?²å%Óâg?ßڒfçý?²Ä@8Ã?ÍTÇ.ʐ)?³>`j§Re?Ñ{
aF°­?°©qÖفkMIXED4FGL J0135.1+0255?êó•I¹îŠÀM½º
RiÀ;w³Š§àÀ<­ÓÀÜÕ@"[ÌÚ
Òü?ùYÝÿôB?ÍoÃ\`©
?´~!sBB?éSme^(ª@(â@Q~οïþš9҉¥¿¹³BVä?ïüùðòF¿Öצ$lpì¿ïé
?ƒ£Ž?ïгâ;ëAGNbcu1RXS J013506.7+025558?ï×I)¶ÿþ?¡BUÙß?C,"±ì-?udI¹Yñ?qù¥¬ý–?œà©·"?ïÕ¶š¨¯®?yH¶é½É§?B•9
?R¥QS'÷?rÒ¹ÔË?v†R5º÷?w×ä?š'5»™!?x1ãuXcC?!äñ¤¥?¤|u1é?™i•ï
Ò?ïn4Ebh?w'Ì£`Zœ?BE‡ø #?96yç
?'¨Ýqo4ê?v횸SŸ4?ïË2_gˆi?wÐõŸ]^?EßS¿E&Ý?C°ø—Œ_~?wªå¼õΫ?vþ¢ÔÌ
³?&<Äp?Œ¡ù¤+X?Rÿ" ßAB?tX	£
:O?†´éi‰³?Š+>t?î(
°±}?œÃØÊkzv?xÌ¡œ…üÁ?'XM
ؾ?ªfjô
Û?œ¸#(–P?îxƒti3?'·'ËÔ[?N%ðæÍ}Î?Oa̅ªXF?¦àÓr…?'š?ôaNAGN4FGL J0136.5+3906?ìuŠzåïÀ6ðMDVq&À7´åÏxyÀ;<Ðjæÿ@"n×S9?øû"}ö¦?š›œÂݤz?´û0f…p@Õèc+Hƒ@uU6=SÈ?ïû!>>)0¿Ë»Cs¿×Ëw!ʀ¿ÑW8 ,ñ%¿Ö˜Ç¢"¿âCÖNUÎiAGNbll3FGL J0136.5+3905B3 0133+388?ïDçW+yÅ?›4Œ€·Þ?t+àÊ­Ó*?'+šêÿÌ)?'Xîð…†?"˜Œ˜)?ï"%¸²?‹ŸÑÊí·?b§1%¥v?j‹❳ ?†PO¡ôt?ˆéèî>Ø?ìZ0ûv?ª®
i*?žXäà¤Kø?˜Ò
½þ‰Ð?µ˜>ífûV?¦sª8üŠz?ìºÿ¦¥?›­úüvc?ƒ†Z(0?k¼Ý8¦Iá?··@¿$ýí?šÒdu k?ï^! 6+`?"U;‡Ù(?mbÂV"î?qôÅÁ%å?˜?Õ~?<	—<ú?/ÊaÒ?©ÐMT¯uG?ƒZªüY‹™?š¥r_î? ¿bAmÒy?¤ä¦p¶?ì»2êFì?ª(AB¹¹?—i67*¬?" Ǐï;?´L)*²
s?¦þ¶á eÞ?êÇŕº¬?°}";ŒÇ?ŽŠ¸Ã:Ù?~ŽÑÍ
J?Ŝ5[½§&?°³ú†ØòAGN4FGL J0137.0+4751?Ú:ÔBYcÀ,žß?–À8	wíwg@À;–ϲZZ¿@"58$t@'ßƤ"Ÿ?œºâ"Š;-?¹E6€o§@Ÿ
âµ@¹õ"¦î¿É8ÄA¸Ý¿àiˆ†a¿äªg|æÛl¿ã÷±j8X¿é!ÔfB¿ë|辚ÚâAGNfsrq3FGL J0137.0+4752OC 457?ïÇ@mQß?ˆA0HÏ?O§Ù¥ÔÛ?FX~3_Šç?x}4VDjs?ˆjIzu?ï࣏k•?sr†ÃÃú?AÊjŅxÐ?XD$y\d?jéÖdzyÖ?qIEmZ?ï̽å˘½?qLÀˆ%êÕ?`ÿ[H&è?lí@Öû÷ø?q!_ŠÏÞA?b³p:¾­{?ïó¤ðîGÏ?AÌNQ&?1ií-}›?!yu5+ô?T[¢4t?>¬÷–±tZ?ï¡#}3?zc"ŒNÝ?Rx-ñz`)?Oó`áÛ°?…iñ''U?xÖb
(ÓT?ﵯg®‡?'ÃßÏ>?Vó¦Wy'Þ?uêt'$D?»¾´:—œ?E?ÛD*?ﺔp1bÆ?~F·Ør•?j¥†xÞÅ¿?vL£S `?uc'"
N?q½ÓȎ?ïáSOê|?^$'·îF?D'Þvm¤a?8
6'†>ß?i‡øÝûá÷?['Öçåx\AGN4FGL J0137.6-2430?î;)öTVÀSÒaAcwŸÀ9ɇî"À<BÎxžw@¿aj~#@@E®_ú?¨£,ëEˆË?½¨Ù'¤Þ@«c|§Œ@[òPêԿž¡{eQ¿ã2†óпçWã줩¿éž¥2¿êÌÝÿ$7î¿ïÿŠYŠµÑAGNfsrq3FGL J0137.6-2430PKS 0135-247?ßWò'Ø¿¨?Þ¦nIÝt?6*Ýw‹Ä?>ƒlf3Ó?àQA}Þ?Þ«Î E+?ïêhô,¯ƒ?iëÃM£ô?2"׋ãk?CÀ;u§ùÃ?cDÙџõ?gCü»É5'?ï–
ü»Ûk?ƒ{¨Ä#?spÏAg?Oûî0öF?€ÄÙ:Òº|?xE"ߺ?ïü%#"Éj?#)…Æïó?XÌÕ;jŒ?ûJ[|yð?7@°ZFL?9.–¤?í* cHŠï?ÉJñ'†$?UOp/"ÔC?zP~³:Z¿?¶U¿%Œ"ó?É'~Ð{¿$?ïÆ:Bà¿?'§«ùk,ô?KŒIp˜ÿ?f¸ºÝ•?yqUvÒà?€¨®FF?ïbÑ3ÂWÜ?‰½òª©‰?yW.ßSý?ŸGŸ?Š £Pzâ?'3(B‰¨c?ï÷u8LˆÖ??{5áºé?1Y7
Øí?% Uçdg?I~^+Ž·?9k¦‰­MIXED4FGL J0137.9+5814¿ïA/¹ðÁÀFïÃqÚ8À8Î3œ¾àÀ;ÊÖyù@ -ÐH'OÑ?þø–IƒÑ?¦ZßZÕ?Žà8±Ä«
?çé‡=G@úºÈ}Ü¿èQu¾sпԳµ'k€¿àħš
\à¿Ý
ˆïþ*=¿àÅ+<¿ØO*ÀH&AGNbll3FGL J0137.8+5813TXS 0134+579?ïÎËR¾?hDuÇ͟‰?9Ƭð¯:n?,E<²õ?wY¯†Ybª?gB
!{)´?î) ò¥?¯'•êô'H?A«\"å­?R<3·n?­)€o撨?¯_ª*M•ç?ïþ«?Œî´pbþ?iñH|n"?r7ÑùíwS?™a^	¬Ø?Š"߸hºõ?ïxšæ ³i?qi°µwk%?\Ä{
ø6?@Ã}1õÁœ?Ž@·âv?pgù©›ºœ?ï‡*r´a?ƒZ&ƒù§}?M`hm×ò–?F«R"ÜÉ?Œ_\ÁRï\?'eOwýá™?긽aRˆí?Á.,/«5Æ?Rº~ÄMò?jfF4›U?Ä÷•xLÂÑ?Á$;º|y^?îjh9?"'$j¿ý·?hGVi
àû?d%øߓ	?¥«Cøî·Û?"Rî>«o?¨ë""?‹c(¡èP?s-$ä°w?^{Ð
¬i?¢qïÐC5?ËöîF_¯AGN4FGL J0138.0+2247?·Åbª'³ÀCi:2?îÀ:%:G#«À<R÷eýŠÛ@²xà;"@}æOU?¸6Îs@–?q8áh¨E?ºS²ÚˆL?@z÷NU£?ì³åªê#ö¿ç^æªÄdH¿â ÿõEq¿ÖÄÀŽÐ軿äy-Œ*E¿ËgIû¡¡{AGNbllGB6 J0138+2248?ïõ:ÄÇ?K<xKB›b?% :–Œì?ý¡áÓ£b?RçïWÜï?HŽÍ6¡ï?ïæWé(«£?j6ohì?1[ÅÐd?@y`Ì®?g|žq`ý?g@Ðjù5?ï·[¢yMZ?s=d¾‰PÁ?K]ÛºLep?2"U¿»?€s9¨4¼?sìø:¶?ïÖ{·'ìP?P½¤1îO¬?9»Å?y?4Y!??s0ÓT¡Ó?P1荀äý?ïì"Sð©1?T¯ŠÏ»%?5>ˆO'À?(n–aÕ ?`ÃÚÏ0·¨?Rʎؖ³?ï´«bËÀ?'‹uòû?8èxÀ?Hµ¼}/Û?'
ælø,?±r_E>?ï{øP€˜c?÷n$åh?T9¼¬q¢*?U0.·§‡?Žz´X
"Ü?ÇlBúÎ?ïŒsœ§8?nßv%U5?P¡OabS±?9Æ^‰És?Šæù49?n¨CÆ XAGN4FGL J0138.5-4613¿í¸";¥ŒÀQ0DR?gõÀ:j&Ñ%!"À<¤×%+3@îrì û@î¨|‹kÙ?¹õìUÔ?œ'Ý<Ü?ãªJè\?øs™)Ý?ïï
3Å)j¿¹ß#¦@¿çǃ·°¿Ù@X *,y¿à9¢cÑ¿ê	Ý>_SAGNbcu3FGL J0138.5-4612PMN J0138-4614?ï–ô<
³ƒ?…ð²f6n?Rbw™Á"þ?U{'ªõ$Å?‡ö¡øÜÌÔ?ƒzvCE}?ï'ZEEÚU?"‹ë,ë?cwŠÆ°ª?k9Ñ|â?†‹Œtm—?'òÙ]øÛ?ï%:Ý ¬ô?‰ üõ•‹?y®T
Gs?€tÛL«úü?"íbs'Ÿ?'ÛB^.ì?îëѦÀ?~3P '˜Z?'±åo?jKZxôÁß?™,؟?«$?wÌÿ>8pÇ?ïN*IÌõ?Žl3.?aʤ'~?XN«vË??"fàÉSÓ?Œ¨íÿµGï?ïŧ¿w$?¢œ¹Ã1wÚ?v¯ðÿú$3?Â‰¹

–?™ûNÏͱo?œ\ ­ÃžÛ?ÞUÙ?'àÉZ±º=?®×lV¡?§St#ñÕ?¡ù¨Ø8×0?d#|¸†?í)\ͶV¿?–ÇÒÝ 7?™šàd°ãö?‰Z|XÚ
?°NaxE*?'°U"Û]AGN4FGL J0139.0+2601¿àώP:UÀAϋ«`kÀ:´•ë/³À<8;-Ówâ@@,ôÄ0@"ÅDBO0?Í_á'¿'Õtß'¡?Íw,‡G‡~@¡¤ì³òá¿ë>øcSŒo¿à_*g²–Á¿Ûétƒ	µ6¿èBÜôb=¿àÒ\XÆ¿ïþ­…èÝAGNbllWISE J013859.14+260015.7?ïçxúó@?dp+2ê?BuòPt?IS­VÂn?d«'íÏ?^ª|Þªr=?ïÌ8UÅ?qªÃfÀ?C'<ڝh?K?!ÇÞ¢ù?w~íÅ
£¬?nÛ©-f7¾?ïá…QÊ3?€vöCëŸ?gî¼G®¿??sT"siÑ?‰‹ï‰{™r?zÖþ¼Ê?ï Ä"'õ?a¬Ó3ùi©??ò£êä™?%¾%QÚÉ¡?†ÏIîz`]?a"— û¿?ïÉi3±n‰?qˆ= Î?RÿÛÃ6ØN?QjÀ9×Â=?v‹o-Œ	¡?l
w—W?ïBü|ÆWÆ?—¼šÍ¼?Ut Ã#?`ž¨Ê«‰­?–I.Í;ë:?–ÿa®øyÄ?îþa!ƒ‡?(s¤'úÈ?sLƒ½?‹8?wc îX~ï?›`ºÙCù`?‹<(>&p?îäïìC?'sò->˜?VÜyà.
?Gy6bwà?¡48(×?'?COF¢nAGN4FGL J0140.6-0758?ë'má@2†ÀPäýó¶E¢À;¤ÍªB^À<™€'a–ô@ ÁŠ^"3N?ú¦¯ç¹¸?њ'ÇÅý?¢nªW¬å?óÝ­ûPm×@KŸ	0¿ìèiÿ#â?Ì:OMw¿×wS´Eí¿à­'f¿½›Á'¿êøC""~AGNbllRX J0140.7-0758?ïâf0Olé?[C%
÷?3
ý
 ëx?%9A5<¯?k8p,¸m¹?Zz"|Áu?ïᵄ(:©?pÐԈËȘ?9"DD[Ê©?G¡ÿ$7§O?k'¿?m…Çé"ܨ?ïqŽÚV?vy¦°"'.?W/>ªµHÀ?B‹xÿ+Í?išAmQ?u¼ä‹Q·?à¿{‰?dþùÍõ?4åv¿gLà?#Ž.¤ùÚO?‰*\™|É?dœ­Â?ïÄ­5¯x?m¡g}Äz?H̐
Õi$?>Ø$eÝ?zÓr…dù?kV³vª£M?ï«6"çƒ1?…îRç*1‡?Há/½Š$é?[Ñ©2ÅKb?ƒ¤GΚà?"=¡Ö§?îòYÜÀ5?ŠÉuTjæ?a(OOT™?aYãÐç:?ŸŒïÀ_È?‰9'Óï¥?ïÇI«?'J#S.Ë??yà"<=?7%ޟÃ"Ç?Ÿ!'>!?'@'kKÙ?AGN4FGL J0140.6+8736¿â
ëøm@8ÉÒ¿UÀ:ҏØO·ÎÀ<A(¿<@ ï>fÃ?ÿy)L)¤>?Ç)×iÞÀë?¾ä0ì†ü^?ö®×ï?¾@
ç¿P7zì?ï(šÞ"ԿۏÔ>0<^¿Úõt,öƒ¿Ü/ö$_¿æ¾­OY§¿ÑHÈÆ­ÎÛAGNbcu3FGL J0139.9+8735WN B0126.6+8722?ïðœŸ!\¶?HÞlL"ÔŒ?0ÀápA(?$ûv¢Ç?Z–‰&T\‰?F‰ØŽË¥?ïÎñím¬?p~(Þ¬*?I=—Íá?P¢Å%?u×ãÕr¥É?l5
šÓy?ï»­ú"sT?g	'c¡±?O'òò>?5=OîM"?~8°À8ª?eßQq¨2?:/ëo?fÚq°±`"?`ÉúÜáŠ?;~Z
‰Ãí?‰cсTÓ?f‰K©ÝŪ?ïåؼÅÍ?WN(Ôú?@ž‰LD?6ÇQdcY?eÿ Î%?U`
ú«g'?ïz~µ¬c?‰Þx(­4?YÐ1ù1w?b+¾B›?Ž&LfeÛ?‡7…Zû×°?ï…ä×&©?wú"D;âc?YwT‰«K?^Ã^ÑR?‹XK«Â??uˆtïpY½?î…ã6úÁ?"O	e«=?vws§‰Â?\¾…¬ê¾¬?¤ÒÞ¡
'?"D¬3ýkýAGN4FGL J0141.4-0928¿ÙÔÆ`¢GÀQ1=Ùb·À8wŒE@ƒÀ;¯p"½'Æ@?mà-QÈ@²ƒ\@s? Nší¬–L?¨]ã#ë@ò*ڟg@0;'b|¿´#ŽûZÿ«¿Ý¡+>E[¿ãÓþð5ˆ¿âh·¿I~¿äàӟ¤Ë|¿â#*!;¹êAGNbll3FGL J0141.4-0929PKS 0139-09?ïô/ýž¦Ê?FŸÿCuÀ?íéõ°Ï?E*,ͬR?UÁ%ø€»l?EylDŽ~Å?ïðõ|æ¨?cjð÷<ú•?'' ùÒ?9íÒDa~?\åïÚU7ö?aM™±"`?ï·MÊN ?uMR•
€?YìÀiÞ\??eQ`˜
Á?}Þ@"ÿÖ?pÕMã?ïôÇXf?>Ü4wïŽb?8ZIRc?ñ(Á~ëK?V'ë–2O<?=×Õ"ÈÊ?ïæâ›dº?bÔwÆHä?#dÀ+Ñ*…?q²!ày?h"¸kd?bw#þWùW?ïÐНz`?€¼\äá??ðq
døõ?Y±mžá¦?u˜÷¢TNo?}}®öì?ïŽP'i
?| ° Û?aþ"9m<ú?h½ス¶?‡ìTÁ<9±?Õ?ïý|	?ïéui[Ö?TšÑÕ°®,?#µ";êÔ?>$M5bš?eO="…ê'?SîÜÓ0AGN4FGL J0142.7-0543¿âküc¤{ÀPWÁ~ºñÀ;c1'À8À<±ÇÞP'Ï@JB•ü¬@3çÞ¡
§?Å?Ò(z#?ªqáÄ«–?äuòËd@Yï>½?ï÷®»iοä¿<Uñ¤¿ãʶ!œÁ¿è´¾c'˜¿Ëšã†!¿ïÿ~À¥L*AGNbllPKS 0140-059?ïÎÔ6M™ç?~5ë¡ý(?@\Îûî†?9îÁ£u÷?v'ùHT"Y?}¡xS'lÚ?ïՒ(a&?t3k"±þï?CÒ,þbn?OyˆÄå»ê?r¼¦6ÿ|=?qu'ê­?ïslöż?Wç+"(?`Xo6}mO?k2ïù …?¦¡¹?'ÖWd¿?ïص"Üž?So—¤¹=½?0ޔ5óÃ?
(ëžO?ré¼
	Bg?S"IPŠí¾?ïŒùp¢]?…Ph«Ã›?UîÚ9W®?TʍÜ?ŠȘ|çq?"@'`†?ï–Yü©<?Ž
u?R¬ÍM-3Û?bҕ:ƙ½?ˆç:!¿?‹‰›ÂÎ"?ï¿g3•Ú?
Ωà}s?fÞ9ƒDȦ?h¸­6S«þ?œLKã!ZÀ?°JëH©`?ïz¿ú+¶?v<FüÉ?He+Då9s?>ÕÍ?xƒ?É®Âó™?vG@¥Do1AGN4FGL J0143.1-3622?ÊîÛ%2rÀRê–=Ć­À:Ìí¨À<"±ö‡±:@?þþMMf@qßƤ"Ÿ?¶áÓÞÓ¤F?»Æñ@Ÿ'g@.eÙx¬º@Q)¶1Õ»?ï÷XÇAr'¿åÀÇ`QN|¿ç!¼¿ænBÓº&Ø¿ìqT h«:¿ïþ–=Ć­AGNbcuPMN J0143-3623?ïô>…¸Ÿ?H<CÊ|‡Ý?8͸]…?+­²LÞk+?Q}'Ó§?DK'Æ?ïì´]Á°?h£ÂâÈž?1Ä6~–?@Úéä	 z?a[;+®?eŒ-é#òÝ?ᅰ¨Z?qÁ _5¹ƒ?`þ•LYÊ?l·B!¼¬?wµÔ
4þ.?bítpíäW?ïöpl(?5½¸à:Þ?1'Gv­á?5,oTYž?M}G<™uj?3=Þ¡#½?ïëìèv ™?T‡­¤a c?EåT)>?6söGž'æ?]mî€àÀ?Qºéºâ@?ïÈ û³¨?±†:?>²­
é®?Qªaª5?zW¼v0½?€½~XÔ
?ïšeÀN9?|w"ñ¦†Ì?iL¸Äùœ?t0@‡	^?ƒ+¸p/?qÕµ=؉?ïå±ÇQ§?T—·Ç£?H`	°e´?6»æAù?d66CnÙ?QËGžõƒ
AGN4FGL J0143.5-3156?îg,"âqéÀSköU\RçÀ;È~‰rÛÀ<´Zåÿ£º@Eöê,¯@E]D~µ?¿"/?]¸î¿·(p«¯Ç?öî |wJ?ýàÆúOçÊ?ìÒvÅY;¿æ2eByø¿çÅÅqŽ¹¿çš×Q‹
¿ãµíB
@°¿ïø:¿¯#AGNbcuPKS 0140-322?ïķʲf?‰Ï·L'ÆŒ?HBÝ´.›?\ræâ@?z›¾Ðž]5?‡ äM7?ï¶!0žZ?jG˜¯1±?Z•º^W›•?c¸Ú¥k?~Iùbì?|j<ۄ?îåŒ$¢2?'˜²v±Ît?o€tŒÝ?p»ëî?Ÿ^i~#?'Nv^Êô?ï%y·É?j²ºýÂc?d²Šÿ¿g°?Qqfо¦É?‡Š®XÁ®?gÉÑeÒޅ?ïgîûS|?"þ>25tf?bŸ¤`ÃÌ?e£Š—ö¼Â?Ë¿4?"ìºF?ï<™Ù…lç?šê?EÝ|?lŒ°Ïك'?"k~cP?"Û.³siÂ?–2ã˜pm´?íó¥Ëoï@? ˆ•èĀ÷?{Œ­Iè?wûóG23!?­T
Ÿ*??ŸÂVù¢H?î'ÛŸ£sã?Ž,;(gU¹?Q¨uöÃi?s¬Hò±é•?¢øúýv^?‹^WU$ÀAAGN4FGL J0143.7-5846?Á¢Ìύ,µÀL‰A|¢À9	ëîÑÀ;òˎkß@/Y®2'?üz}Å'¼Ý?¥%þþ^{?¦Ì7ógä@n:p>V@Çc,Ë2?ïüX`iLJ¿Ô["©¤¿Û÷cÏ2X¿ÜR²à£¿ßŒ.Â5D0¿Ò6ƒµ+ÆWAGNbll3FGL J0143.7-5845SUMSS J014347-584550?ïÔ?±µˆý?'}£<tµ?pdÖØå?'†Œ»S—?W_	`?Gë¶0:`5?ï륯Ž#?h}À?0ôhö›kç?>_ò©_?b<V]/â?eÓÂtV,?ï£
sÌU"?w	ÐM\Š?\"/Eà+?at#—ωÿ?ƒ¬âya?uy†Ò‹3?﯁bôŸ'?_!ßëæØ?LOõE¸?0Ò®8?'Z§å…ä?]—ëí?ïÞ¢ú¸º¾?uoëԆ à?Wj⬜þk?s\°ìܶŸ?e§"ÄûŽ?Y¸ÀBQ;?ïÌYˆ:)O?zyþԝÛ?>\6³*šI?PC¨Ì'â{?wíxf2¬Ø?}9"~ˆUS?C"?€_c'?bXC3`Ÿ?j|'ê,gë?Šÿèáˆú?}4*Tip%?ïQæªeç?wËÇSz?\íэ§w?I	@¨Q?"ÿf	ñ±¹?vʲ'œ\†AGN4FGL J0144.6+2705?â'ààUÚÀA%ú](ÐÀ7¢½	á*RÀ;[.ÿÇËÜ@‡âÏmý@C`Ðԙ?•s‹½ãÐÊ?µ€À)¦@ â ÊæBÀ@K)<d_P?œº×+öS¿Ûü@Ã>®'¿âIÆ×p•¿áÍE˜…¿æÒí­íäu¿ç³Ø>ð֗AGNbll3FGL J0144.6+2705TXS 0141+268?ïÌ£¨wi)?l–c‡K|Ã?Lg]ä¦?Däë…\?v-žÞ¤Óñ?iÇ-œ("?ïugcø‰$?"®`""8
?i¹Š™¯:¬?€vŽ©·°?Œ7ÄOkFL?WÈ ½%??ïy[¤I(œ?'8`&'á÷?€L#óê1?ˆ.•î°?\òíó`ÿ?"ëՌËE?ïa%®Ýšó?wósÓúý?sŽXHò‡?a?'nQ8Ï?Ž.Mõj?r"kùX?ïÈÜA"ÎÑ?n`%ádT+?Jé´¿t>ñ?Cx-r«]?x4¨õf^?lE6NÉLG?îlAKœ-?ªf¤ÿÈ/?@}nÒb?ù	ÇÄ?¤ëËè箧?¨@€›?ïƒ|~֟´?caI'-š?wö¢H"¼f?'Vz€R4?ƒ%1ô¤?…¥1`à?šHɦ?‹Úî"øÅ?'Ð•æ ¦?t÷'Û£? buqðRü?‡Ž+í½µAGN4FGL J0145.0-2732¿Öù#Õº"ÀS†KâCÀ9Xy˜rR-À<^ûE†@'‹öî´S@×EB<?¯½dác'?¸ÆÌ,¾Ïß@Ï¡·uM@ÉñS"ÒŠ¿Ø?$=È¿ä¦$Ÿòy¿ç»Þ¯¨Ð¿ê˜£?_¼S¿ífà‰Ã
¿î½Þ¨v¬AGNfsrq3FGL J0145.1-2732PKS 0142-278?ïö•_ńÑ?Fßz‹‰y?(Œæ¾p?ŠúDèÄ?O‡³T&j?Dî&Óècé?ïïwäŠ{?dâ³ZŠ6?*ÝöÛeáú?;K—·Çû?]´w‹eÅö?b¡"Žuà?ï¿Í
gë?qI3V~p?[×h½qЩ?e9¾rJI?y¿]ýyü?j‹;rÝp?ïÿ!‰Î±?ÃÖ©Ôì">ê¨`ÞàÎ>ۇL:š"?y±£üÝ?UÒJôŒÕ?ïñ˜ Â¥#?Pc:˜EqO?0ʨª¦ô?$"j]ÂÈg?Xœ¬VØ?NG-íA?ïÔ£ítPú?Ÿ¸k¢?;ÇãÇ|®?YviUérs?sñ‹ýe?|u÷ž÷˜?ï't9æî?z©O$™}?b–½ÈØ3y?c˜¯éÜ	þ?†½BMÿӏ?x³ØÀ(d?ïþü§
©?"‰"·‡Z>ýÇEG¥±…>örÚHߊ?+×I׎Õ'?!ã^™"AGN4FGL J0145.9+2319?êq a}ïÀBì앿ðEÀ:ÏÓØZÀ<[‰2CI+@Ýyý@žÉý³ø?Ç·.jv–_?·jªÃ¸|?îzÜ?0—x@8'ÁÞÝ¿ã7=N?(4¿½x³š÷'ž¿ç=Fý•lŽ¿çLƂ/ð‰¿àɺ^5?}¿ïþP§ETAGNbcuTXS 0143+230?ï¥QVµ?v¬ï² ?E¼ø¸¯aN?6½¿7'÷?…_lœíSY?uá§í…?ïÄàiY,d?s‡ÊÐxqä?H%šeó‰ã?Qøö70™'?z‹ñjº?p™È^@6®?ïa:åPž ?{ó
Û¸0‰?gߍydÃ?c½	kÿ¤†?õ'g€ W?x"Îä)?ï•ÊÒ2ž?b"ÓØ
v?SñÏÀd
?9 3"'Þ?ˆ=!?bã…ðø*?ï!¶ˆŠ ?)µîZ–?X´ÿmŠOU?NÍ+‹ãš?š=Þúû?NÝ1Z?ïDõ^L¢¬?'c>ʳE|?\‡ñxk2;?n´‹Ë@SÚ?•˜Õ©8[?¨q>TÑ?ÃD±?~‹ºø}Ä?t
ÿµ
.?g>šªCÁ?¡…Ñ1R¶Æ?ŽÙLjš[?îÜ:«¢…¦?€æbUй?hՎÔüì"?W º'0D? ®üUœ+Õ?€ƒ"ÑùpAGN4FGL J0146.0-6746?ï¼ÈÒä‹RÀHBòù‡?ûÀ:$"çƒ1xÀ<"Ö«rßñ@#¿ÆÿÙ??ÿD¶Ê,	?¸\ǁ3qG?¾E¿&ñÜQ@·Üz¿¹¿@|š	Öîd?ÚÀïÿÕÙ¿Êèà©£}¿Ûú©ÿÿáр´¿çÊäÊðS»¿àów[0AGNbcu3FGL J0146.4-6746SUMSS J014554-674646?ïû‹W±è?.€évÎoQ?!–'"X"G?í´sÛ¯Í?:Ú=í>A?()UC"O–?ïáÖ<jÇþ?pdÖÞdu?;)‡¸?IZ›¥Ç?jģĦô²?l¦·£ëŽ?ïÇÖÿç½z?k½7á÷4?TòÊõ¤?aè~ä¡|ª?v×ÍzÕZÑ?dP¼ûCd?ïÙËp"Ê?N\MŽÄmÂ?Qª"ñŦÒ?25Ïïm±?néû}'–?Ku+K|ùŠ?ïög˜jš~?CW–|`–?<Ñ{¯-_Ä?9ºBƒ˜Ö'?Gøá#yUœ?7Ç2ÝË"ë?ï±C+†
?"†?æ$?F…5`?X0­
"'?'FG[5>?ƒL6¢óò@?ﮜ¢&tÎ?pŸA^Ÿ?[Í$K'áX?aoº!aÞ?€ß2òÇæe?hX«~"¹¡?ï¡Àd¢Ó?i÷Š×""?cÕ˜€él?LrÄÃ¥€š?'š–M¨Ð?gºúFˆIAGN4FGL J0146.3+4606?å¢Ì¢ý½ÓÀ/j²[1~þÀ:ʄս6WÀ<"Ä'k§ï@VÖüPž?ÿå€éŸk?ÇD×àÒ\?Çaá†îQ?ý¹áˆE´??û™R.v
?ïäY!bü¿Ñ²mÛ¥­¤¿àQøPV¿âÌÅ«p[³¿ã%™'¥R¿åAmž%øAGNbcuB3 0143+458?螺Ñ	ƒž?vXâ/
µ¶?["
Ÿƒq?PçÐú"À?ƒwK´\7?t2ö'èý?ïeœ	
•°?ŠÑŸðJÖ=?q"»¹wÛ?rþÝhõc?Ö÷^uö	?†T<«œð?ïXv$Z¹p?€wöŒ†Ý?rä"܋?t=è±Kf?8:7®Ø?vÁöfŒ?íßIv8
?~â[¬Ã?'FN£ï6?m«fƒL?¨èbyx»?{©5R!&î?ïS\o±W•?†;ÂL5ûŸ?lÊ©=oÜæ?aGwoè?'ûã²ä¼?"D›X-d?î$¨Je?«Ê'3©-i?*ÿþ•8?¢š4þr2ä?¦j¾hD²Ã? ­¾lFV$?îåbÍL?‹'åÞQë–?}åhO¹È?}¬œüw ?›ÚL,Íj6?"€¾®tO?ê–3+.4¤?—3á'ÒÌ?£¯"g¿ôû?‡=%"(p?À»j¸
U²?•æüßö0…AGN4FGL J0146.9-5202?Ô~¯9‹ÀO~÷üü?À:aØ›ïµÀ<!Õ<Ý×@h <K	ê?ÿUûµ¤a?À®I)ʍ?½>[/{˜¨?þ"T8fxÛ@P×8`™ž¿ëc>Ò¤?ÇA»Y¿á»Ëǔ¿ß¥áË·y¿ÞËSûÕ£á¿ïô`{?çAGNbll3FGL J0147.0-5204PKS 0144-522?ïßI[éŠÉ?Z£duTÓ²?FŸ+ӈjû?; ÷¯{Ä?kÙі?X>…œ™?ïÄ8 u¨?}D—'´r?SÌ#Ä}5q?^|L.:P¸?xð°f˜›?wp~Ì­¦?ïzÿÙ¥´k?yüÅÞÿþË?gƒ"T€Å>?gm8Îÿ?‹_@þæ?tNcÇAöÚ?ïP˜õ7'¬?o\xˆö?r«º|<åW?U+f%ûk?'Aò¼ì-?k%œn£ˆC?ﺫMém?nß+œg?^ÿIb{Ë?U	hv›o?zêŸ}¬¦®?i'¹g•?ïK['el
?•f–éº9?kƒ'µ9‰??zƒ…•/™w?"$(¿–ø7?'P?"ˆ?ï*ø_*e?'™1S"îY?qB&*‹É?mÝTpnJ?–Pj—¼©?‰k#!?îdt9Éáq?‰´äÌéjL?ƒ­Dã´Ù?q¡ÈFëÞ?¤Ík(ÿ
ù?‡Ì.±8AGN4FGL J0147.7-1321?ïŽ6텈ÀQ½×¡<%JÀ;i™ù:éáÀ<ÐI4&x:@Ë{uÂ#ü@Œ¶â¼y?Ú#<E*¬|? ú¶j	ß?Ä¦ý/k?ÿÀN²º¢?ïú
'Íx¿èå).‰¿â;¡–¾¿Óšß_ ¡á¿é~lLYtæ¿ïÿúŒ"¸'AGNbcuNVSS J014804-132019?ïÌß&
'?Š9dÞM"
?L´J\k?]ÍÞ¿ÆY?vn™Ý¬"?†½« \?ïÍv§…?x¿©†Ë-Š?KíUmI~1?TÑãΣ<?uÇâ#eQ?tó8ä"þ?ï!Ђ8ÿÑ?ˆÝ–×D
v?l9µš_sú?oNÀ!ٜ§?˜>¹÷@[?‡Œ«*?𥉉UÎNé?d}KV&ê†?O¨r3ºƒb?7Š0×03!?ƒ #[ƒÅ+?cÅ2§¯ Y?ï¡xَ.à?€
Ã^Ý?V³'iØ·k?SïçϟŸt?"ËWrP×?}'îõT¢?ïŠ@Ë¢*b?õ‰dY?V¨ëÆ?b£'ÛÁˆ?Šš¯œ¤á­?Š±è¥-g?î HsÐöí?'3œßýµ?sÎrwjg?t¡ü›oÓ:?£—žö-vä?éOc¹?ï+fg+÷ï?'£­Ÿ+#?XôiFßD?TÛr;èP?™싾k‰?'yÃ͌ÄAGN4FGL J0148.2+5201?ïY¶ØðÀ#¾åGÆÀ9³EB<À<!»¹@ ¹%ô†O:?û^SEÎ@?´lŸe‹u?¹—½÷FóÚ@Tù¯ƒç@FI»_è¿ïýè~;?ïÿõÿ 1#¿Ä")Èü3¿ÜX
Ã}m¿¿Û¼ýÌÉó¿ÕÅi@¶SAGNbll3FGL J0148.3+5200GB6 J0148+5202?ï‰'ÿM}Œ?†p-ú	'
?QUòèҙ?IéA;ô?‹‹AÎ<ʝ?…qÒý­ô?ïW²1å¼?œ#^¾w*¡?UU4éÚbV?b	Ü+ËD?"´YüøE?›'6tŒ?îᄀòr"?Œ9KÌ×?t7õÂ;ݧ?w€U'‰?žÁrt¾M@?‰âaù3!?î"
ª–?zØt.PÏi?ƒu¾¨#?e	`b֍æ?¡á﷝
ž?v³fJH?îœ~• '?6¡èø›j?n‹4à]&?nB¯«?¡í"ÉÆ
¥?›N×å•Ø?íé+`3¤ü?¶§qˆÍ?q/sM9°?€ñx1xË©?¯G["hfÎ?¶rC†•ð?íEmé=÷?Ÿa>·µ^R?'Œ£jÀ?€S"óãÍ?³'üIª'?»ùüìá?íêL˜¸?"˜Ûý˜üÏ?'wÚfš<"?{˜k3¼-`?³·tÊ8?'eÁ&°«ÊAGN4FGL J0148.6+0127?ïºrahÈ
ÀM"!ÄuæÀ:q'ùCM]À<e€<ÑA§@T˜Û-¸ @Ê¡C²x?·­®¤m³¿­Œ^Æù"?öq?|Ì@Ãú³ºØ?ïzÁҝÇ&¿èmÎÜd¿ålXï
¿àæY›|Ȩ¿Ù¢†,Ù¿ïú?̞©¤AGNbll3FGL J0148.6+0128PMN J0148+0129?ïÛ:ûÃI?e‡§è{}?A¹1t~û8?6€è½‰æ¹?pD¼UWá˜?dº\Ýþ"Ê?ïÝü¾rä?nIi‡Vkµ?:6 Á|ý€?A@à-ÕO?n½7öìÑê?k˜¦mP/)?ï—O¿Õ?q´´PÌŚ?Wôƒ?@μñèÊz?‡Hý$!€*?pôçiwe,?ï¼KÃÌQ?^˜3EU?MÌ9µX!?3ãÏõU•?~8™ÆÔ?]́8&õ?ﺖ¯.H?q¢}*9šÄ?U2ìàÂ8Ñ?F˜lj¢}?}gí0ŽÍí?oºéößz?+¯õë?†üœ'm?J÷/|SØÊ?WfåE?…c'¬P?"ú
Ù³÷$?ï"Ù	2?‹8OÜôþ"?evLúbéÑ?b¦pQ'¹?™
[>\_'?Š+ž÷ùâŠ?ï0ÿ¬'Ö?|o¦]±¾?h8+³i¦Æ?XL&¾é?–Ù
‡²N?{^úáÛñ9AGN4FGL J0149.6-0734¿ê¥ue»NSÀP… …±…À;L;æ`ÊÀ<§Ö»cý@Eûxö@Èïþ*<ê?ÒEè8¹?ÃØEç?ê§?ñ"ì~Bûþ?úü,ý~?ï³@S'D¿Ë»5À¬-¿èåTƒ¿ãÅ©!ÌÙb¿ïþ
¡ÿÏ¿ìRÍAç«öAGNbcuPMN J0149-0733?ï–KEp?
àҋþ#?aÊGpá?Z›[9(ï?†¼A?PðgÄzè?ï`ˆ™<?'ÿH'Í:¶?vĈj#2«?Yþ앵?Œ{•~€.Q?‰†P(Æφ?ïû¦m×8?ŠÙVéˆÔ¬?|ˆ´´È7?}›è.J<?•þ^/N;?…•Ñî1¼à?íù¡¾Ï+?ˆGA­ÖYÂ?l½¾Hó?pÎïÛˆ?©
¾¶8՗?…T5͜t?ïIÅû¿?2֓‹gÇ?p%Rŏ4?g–Ã`eµ?'¾e7Î_?‹(¿Z×
¯?îpÀ7b˜?ªcñª?ˆÒwëûºl?•}Tǜ?¢¿añŠçè?£/æ\÷Äö?îzîÑ·ö¯?"kR˜Û?‡Lw8+ü™?"–4$îΊ?¢}õ	JÞ?ŽœÚ$VÕ?êŽNîƒ4?¢‹¬RüÀ? RÜž?ŒùŠh¿«?Á¾

Ñò?¡ê…òØ+#AGN4FGL J0150.6-5448¿ï_†DʂÀN%db€'ÙÀ;K¹Z)ABÀ<ëªfpw@ #Œ¤ÄS?ùÃԅþ²"?ÓñýwŠ%?Ï*y¦41¶?ôm3	AÈ?ýî¦un¿Ò‰÷Dðtó¿êÖc"3ÖÇ¿ßü^ Ia¿Êç‰¼'¿çÕT{ç¿Àψ=üÞAGNbcu3FGL J0150.5-5447PMN J0150-5450?ïÔ~6睴?b®ÚZÁM?@KG2m?.][9Íʞ?s·{µ¸ž?ale+šaç?ï²ðžŸN ?{¡%õ?Y±'lö?`¢qžA¸Ì?€
¨Ð@î?|
¬þà¢?ïD¸F-
û?"¦Q¥ôwµ?kÆî+a@®?lƋá;¤?"ð|)¦?ƒ*[,ÓF?ïFže?tó~üƒ?`xQeBbó?Iý鳄<ã?›("':?t1bss²X?ï¦=ë·¸W?wÓ
uš!?PR(<éL?AUäR.Í?"fBh?vNŒåÇ?ïNOñQ]ã?"…Ýù:¬?e¤ž"Õ
§?u‰­›â§³?"n•`è?'"<ÛÀ•
?îÆ"Ì¿?'Óp™´á?r­ô€T(?sac¼Uê?¡N!ôb:?Ž²øg¿Ò?틙Yéçv?"-íp0j?k¢l¶h…›?an¢¥$õÕ?²Æ!ÊX'ä?"²®åògÛAGN4FGL J0151.0+0539¿Õ3µ¼1kÀK—þŽæ¸À:Á'ï2RÀ<mwVx²™@ӀÖ)Aî@ßûH
ZÍ?»ϘY'º¿²à#–³
Y?øq‹'æÎ×?þRP6ú*?ïú¦$¿ëÆíàBËW¿çt‡>.¿ÒbÌéR>'¿Ú§½ž±†u¿ïÿülòAGNbcu3FGL J0151.0+0537PMN J0151+0540?ï«ÔSB¶ù?uº4¿†Z{?Q!Z¢žµ?@ƒªv?'æ¿élÇ%?tÇz«c¥?ïŸÂ"Nßa?'Dà¿b?^6yúòï?aYÐ¥Nú?"L:•o?~´/&(u?ï/w±‰Ç·?…®]pÕrf?h¿Ôÿéµ1?c*±pª?–ù-Áð€?"'å±H?ï¿MCà?z?tùW?ju™ðæŒX?U*Û÷K<?›¹c?xʁƒ¤@?ïRP,Æ»?Š¸Z«	h?dïû¸%?Vå™ÝlCS?"‰ò?‰+•å†?ï¼q­8Õ?™ÊÛ¼u¯?jÄE'v?tíFǗà?™Ïé؁c?–ÜHT}fÐ?î€qâÆ^I?'÷¸óKó'?s˜¤HîŠ#?lí•[ÿª¥?¥…ÍFà³5?'ñl	*±?ì½{ ·?›^­4
?ŠR#°«¦Y?Xèx˪û?¶Éއ"œJ?™³?Ø¿¥AGN4FGL J0151.3+8601¿¥gÏ6Ó^‰@7GM3H,À:´4çhÀ<h23Xòà@b¡…vL
@BLƂ/ñ?¶ ß´*·?‰0QxåçG?θÐV<<@Ee*§¿çIpŒZ¿áoáÐêê¿çÞl²[¿á['§åŒ·¿ç;ØÞ¨íJ¿ØÖ^¤ÑAGNbll3FGL J0145.6+8600WN B0140.0+8546?ïéw<nè?SvӇ#?@ä½}X
?.ï¥CÑÕ?bO"þZ|Ž?QOîÜ=lk?ïàWbVP3?pu´(oô?AýTÄM5;?Oê
@A·?k)H'Ü·4?k5)‹kc?ïµ+hí?r\+ÖÕ^?VÉÄ{bÖs?`û°çÿ,?·ÚV¶
¸?l	÷›œ™ú?ïÌŽž5W?UK²ªe…r?YëC_ò/?:B(@lÄJ?swgåGe?R"KI-?ïÈÍ<švJ?hLÚ^½Èö?Sé*óÀùÒ?AÑsz7x\?vŸá6ôÛ?f©caX?ïœiˆȈ?†0Øhvø?U(%sç?b©=³5=L?†B
Bh\?ƒ…,¿™?ïm¨w
à?€¨@mYÒá?b¥ù"©Þ?a8zùN»?ìzôLª?}ÒÔx
¿ô?ïi—
ž§?uÖàÇ·e?sº°¡·Y?[~}™°?‹¼ådxn‰?ra"e9™AGN4FGL J0151.4-3607?닫†oßüÀR™—_,¶AÀ:Õ,D,À<Â(äû—»@ʆXõµ@ü\Wë‰?Áú"³Ùa?°ÔâšêQ˜?ïœÙŸÄ @ AO€›Ç¿»,€¼}õ#¿Ü|؃9Zë¿é§¢pØ°¿ÚDí$±W¿ê>ku™à¿ïô¸~Œ"
AGNbcu3FGL J0151.0-3609PMN J0151-3605?ï¨áqZÇ]?u®(|Šçè?^!fßân?P®Í;gI7?'vÎÆû?sŽ0 ¬ì[?ïÅoÎoV?yX{]æp?R·ê¾€~?WB5ä!Tõ?xÆjá¶ðî?u¬V°õ?ï\ñâÓ@Ò?mä㰛>?q2kè|p?r®™"¶ìì?÷f˜º?|"òa•?ï™ÿ@΍}?eo´SfQì?k2úE,b:?P.v*öuà?'³q7Iö?c z‰Š&?ï6öA˜Ú5?9/cªPI?tõ¾só¶©?lCκLg?"ãÈ3Wg½?‰òêü_Lò?ïZDíÎWÅ?'xÑBÀSt?cb•€"D?n…zîiÈ?'K!½dß?eZmvàc?îï9Óq"?‹Ñ{¸Q""?y×f<J¸#?z5e«p©?›¦¿0§É¥?†³™ÓƒÓ½?îðÔ$ɧÃ?šX‰k'?'ˆ‡h<?n›ÇÅɜÅ?˜¡n$Jâý?~®¨2`ÞAGN4FGL J0151.7+5455?íþÔq[âÕÀÀJÕÀ:{93'uÀ<)'(±Ïñ@x97Úû@ßçžà*x?Îû"áN?ÎgΛYa?ñ"ÒTÌ
/@ô"µÜÆ?¿¾HyìU(Q¿»äqY3¢ð¿ä&&À^)¿çO[½•ø$¿î,¦AÕÏ?Ø_`'÷–¥AGNbcu7C 0148+5439?í
–|6dô?©øW]?}Ҋÿ:?pÉõN[?µÂN÷7n&?¨ÍS,
TE?ësqŽ:…?¹¶±ºX?iãÝ*U"£?pOp•'9µ?Áʬ ¯Íã?¹Q¾†ê¿?íå]´*w?še2$cŽO?…Žøpó"?.¬¾Q?¬FfÀÏ©?—'¥&-?ïe@?Fx?jÜ%MÊí?leÿšFÁ?LAñ.YnV?–p=u?gRÜIV0?çšš#ñæ?¿á"n(?Ž}Õ^dæê?€¡w{ºö?ϯ¸Aöx?¿7öHh›í?åßnFspª?È®'û®É?x"ØÆ¢à™?"ŽrâCÙ?Óà˜o£k?Èo{ÚÉð?ëM_adsó?¨¾»h֖?˜†u†Xa?oú—hðb?¿sg´LÖÑ?¥Eµ~Â÷¹?î=­ ÎÆf?‡ÙlLÂ@ü?Sâ9u^}?iš%ÈHÿ?§Ð5cÄ]ƒ?…ª‹»QӜAGN4FGL J0152.2+3714¿ßeÉ»þÒÀ8Sü–ÿÀ:¶ÁȌÌÀ<†xºüÀ°@‡r¨¾û@e%îÇÉ?»üžw?³£çÑ5Z?ñ¯Nìő@ކÀùÚÍ?ïBUåæ¿ãã/áD¿æ³û¢n¿áêP (êZ¿æ:D4w¿ïÏöbreùAGNbcu3FGL J0152.2+3707B2 0149+37?ïÜ£ólâ?nz@%©B?BÏYËc¾?L_ýŸ¿E?n¨6sd:º?kdÅv÷,?ïÐT‡uj?ptmª?DXÿ¬Ö£,?H'f½ùÉ#?uJœ¤ï?m_ê£XÔg?ﲑ7ý?s†ÜÞÖÐ2?Rjp#»i?8ÃÍÆrˆ'?l‹`Ê/?s=tKt§+?ï²R1??Yó$òH|?[cc²ðî@?8sF"O¥?þ"ñJ"?Xµ
¾Àß ?ïTv­dj?²«jdÖL?ƒ+rãÔÑ?²«¡†±·?‡¶âz•É?'n†…%…?ï€[>PY?ˆž¹Úzáþ?R›[_}??^ê;F¡ÕË?©}ǓîX?‡£$O+?ï}õzÈ?[.ƅ??`ЭoÍâÞ?cNM.T?Œ"—W^±r?©Î"ÀÒÌ?ïó¸æ?v=j='S ?sí °Màë?YÄJq·2?—f ÒOÆü?u&߀—4AGN4FGL J0152.2+2206¿îo[»p6§ÀCM¶¡è´À9²j²üA/À<7Üýœxq@Üωë|@åO±;?¶Y 
ý?¾µ9³*q@+ÞàˇR@[Õ¿É¿³Û÷žBÜÛ¿æOâ+ã	¿èÞÙ	1µ¿ç'Á†¿ïÿùµc#¼?êL»P£‡AGNfsrq3FGL J0151.6+2205PKS 0149+21?ïõ©ãX?JU	î&?<·ðoh[?;=^%F2·?M9Bàj?@ÉkQïßÒ?ï'h£¢B?'·7å¨7?f§{qo?|ÄÊ£ëj¼?† -TÉqS?‰î²ø%Æ?ï²ÙC}®,?vë«j?d&_SbS¸?mês¡ñU?|€.yë|?póˆ;÷?ïÉÀÛI^»?[£0]I>?\iìÙ¸½©?D-°7…w?t??V£îLp?ïì>-HŸ?]E¹¥'õ?PI€Å5¤?T2µԔ`?W:DuØû«?NèØ?î˶­-[?§«Š?yś.\ó@?–ˆU—Gñ? ë Ácà?Ÿwtšu{q?9Uü?~ŠÂÀ÷,û?m²sPøʐ?oïuè"='?ˆhœ¦³@[?wQ_,F?ïAùF˜?ƒ¿·ÃTÄ?{¨ã7>Ó?ms4"?ÖØEO54?z"ݘ2
AGN4FGL J0152.6+0147¿i‡X˜UHrÀLÅM@$³>À9mRj0'À<tBÇü@%L=gµ?ÿñ|D=?¯Çˆ"9¿ƒgáfÝ?Ôi,"AC@	B1}Ñ?¬¬j_Lõ/?¸I*ì<ԝ¿ár]ëm¡Ä¿Ü"í*¿à¢¸'¬eN¿ÓVPn­\ÅAGNbll3FGL J0152.6+0148PMN J0152+0146?ïð:ÿ5w?Tm°¤!ƒÆ?/n:ï¦@2?"@KµÂð4?[ž0¥ŒÞu?RåHšlí?ïí<""?hèh{*ú?/y ³ž?@¿2éþL—?`ËÚEÉ?eà?nø²?ïµÆûžé²?u€!x¼Š?Qráæcȏ?:í¬gÛ?€_äæwÚ^?uD¶ú»»?ﶶ~¡Ç?],ÐÚÙÃì?P´
%y'?2¯ziÓ?€;ùbÒg&?[,ª2ö?ïܦ­€ø?g)ë5"?Cu'ª|;?81çT±C|?n˜ô˞ð`?e,ó4d\?ïËå´ORy?~¦6µô™??¼ZÞ2`n?PD§)R?x`2Y9?|V"t¼?ï­Àu¯?€…ó|hv+?[PFc7`?[Ót%՞K?Œª‡"£þ?]}cúÌ?ï]MòbnÆ?v¤Œ!C?b´
ÄÔÓ?M{
á{»?'ýë0m¹Ÿ?tîÏ5¯AAGN4FGL J0153.0+7517?Õ-Pèr<*@)É%x_.À9û)=+ÇÀ<L"4­†¶@ TB…Þ?ÿ&ò³c%?·—MŽÿä?±BZÃpÆ?øln¾#¼ž@$ìH`¿èK·ùÖñ¿­Wåš#,¿Öþqàm¨¿à(l/Ô¿à{'{üP¿áÍ´ôhó	AGNbll3FGL J0152.8+75171RXS J015308.4+751756?ïŒ)ÓÛ?ˆ;s>S1\?V3j¿RB?RK-2º¨¸?Š)'Esnæ?†kÙ·ºï?ï)Aœ"Ó?•®EŒÌã?s=σµPŠ?uAœq?–Zg`©'?"¡Á÷áÂ?ï3
ÔøÈÝ?'[}}H?p.HF!?k¤1Úað"?•"_ܞ!?°xÓ°Q¦?î£Iàb›?'N†[³^Ú?'9÷ÆÁ2?kîñ<©5¼?§(ςÙB?0Ô¹"…?ïQEAþ}?ŒU<&ß®J?iøá»ä͖?\à\E?™Ö»&öÓ ?ŠÙ!%÷O?íj,Óû?²·ºÒr÷?Ž`"€°2›?"'ubÇd?°â†Ø­ÈÔ?°èòՄˆ9?îa»½—?"Õ+¸aþ?x»'Qpao?p°V/¿½?¦ÌÓد¯?'üºìž¥ý?ëÈ
L4?šlë'j
U?¤
8?ˆçc̺¤?½Ó5iÛb?™yߎB>AGN4FGL J0153.4+7114¿ä]+ŠzöI@!ò!ȧ¤À:jfóT À<O$V ž@!"U©€Â?þuêMT?º$ëFàd.¿'y(_ð€†?Ú©=;äó@:šþsì¿ïûÔ¢.=«?ïÿIŒ;F¿è€§?tŠ¿Õrü øH&¿Ü­ÏÜv¸ï¿ß{"¶
nAGNrdg3FGL J0153.4+7114TXS 0149+710?ïPå¦™–?‰y¼ùRä??SÆ;¾¹M?G79yÆ>Ÿ?"¦çŠé'¡?ˆ·°a~˜?íiVcJ8?¹^þƒ2?bÎ-…W+?s'qSJ?´ £ášÃ?¸¯'κ³|?îLDÌ/:x?"hú	ú]?lïh·[Aá?`B˜úäíh?©l¼­û
m?".I$ÈH?îõÅ5mŽè?}DÉcƒÙy?tcK…¸±Ð?WWÑXèÆs?œ.†v`u?}ÁŸÓµ–?îKªk‹ä? \"Ã…•?k`âîÍ'¼?f֊oûA?©Kúo??ŸqÖÔZK?éÁ¢«ÕË?ÇÒò$—†?k Lp+ñ$?{Ë_\'r?Ȋôd2ô?ǟ.Ð^8?ë¯ÝEjî5?¥Biê¦è½?|6Huìi–?p-þ=L¯Ž?À^ئRm>?¤ïŸ¶§?íâŠýß?—7­f~?Žì'öþr¹?y ý²d?³»Ynò0?—¥–	é¤#AGN4FGL J0153.5-5107¿Ç"V)¾{ŒÀO¢sÿ¬*À:Ìg¼§»›À<z9ŠeI@üÖ~|\È@
goF	?ô¹©š¿¯"èÁu?áèæ€Äa@øªgr*?ïøs^œm‰¿éú÷k¿éQÃA2Ð7¿îݼ¾â©X¿ïý®aQԉ?ì!1¾iÕAGNfsrqPKS 0152-513?ïÀÂ}h‹…?Š,Äìõ?<þ]ãÙDÍ?E#!qzÈí?}ÎÛYÕKÞ?‰Œ6-[d?ïºDïôB?†¦od®k?`¶rã[°?qŠ	1˜°'?z'N˜ü%)?ÕC¶/žË?íEnð+TJ?£Œó\t?‹'Eë±9T?°-³+5ð?²b?ƒ?¢y[?ïía¢‡Sò?WlüÕk"_?'ZmGÔO?1åVÐL?a(¶ÓŸM…?U[§;²Ïq?ﺂ¸L|?¬PÖv²ì?DL­‰¾2?YÀµ"¨or?€®ü%Œ?¬L
l©v?ïM¡Õ8'T?ž@UýÚÙ!?q_°æz?ŽÆ>êÖµõ?'e‰l†Ù?•ã¨"ÌÈ@?í¡£þ™ÅÜ?œÜ­¯??'ž¯Öæaä?…i³Z-?°Ÿ
J&?›‡:$ƹ?ï£ÔbI4?•£R¥ËH?@6
 ¤|?^o2Oð?†
´"¬´F?"×ñMr•AGN4FGL J0153.9+0823¿êï<ÏÐH"ÀI°·ÃPLIÀ8ðÑn=À;ª¾®&@7ÕÞCl¼?ý%'6¥®{?¬ÐZ¿6?´s"·e•@Jñ£EêÆ@BíPøì¿Ðmâ;sôn¿ÕŽ_©³Ã¿àlâiø¿Õ¥^~~¾¿â1úï,¿éäÞq9þÿAGNbll3FGL J0154.0+0824GB6 J0154+0823?ïô¤ëîaX?E¹ði›W?"˜Q¼©r¹?µ¦û²ª?Tc"¡àÑ?D#¡*F:?ïÙUK-rK?rá‡_&vw?@¥š·|«?JúÂC¨ì‰?qA¥²Á?p¹X:è€?画<Z¤;?z¼–Wr¾?`^ª'7ŽË?kh^Ç4T???†;
‰?u}ê‹T?ï(o.zÖz?zÌ=§s¬?Xef@æ¢?=02œè2?™póßÀ'W?yw26›?ïè*˜§M¯?Zå±p^
š?2àPaو'?'˜~¾Ħ?ey]Et¹?Y:%P"?ï Æcüÿš?ˆô_7óâ:?Q3	,ù¨?a«±ZÄ?…¨ê'?‡"Ve>(?*^ÖÙ?!ŽÓ"Ÿ?cë/wÛ?k'xÆäÎ?‡£qmÄ1?}™åˆGD2?îIbœØ=n?Àg02D?fÜ«Ol)j?T"ÉUgô?©ü}Ý\"?c	Íy¿
AGN4FGL J0154.3-0236?ïì¾£OŒÀNž¢×/ýÀ:ݤÌӂÉÀ<œ¿eÛüë@| ®vJŠ@É2¼î¥?¼´ßWD5¿©P>Ü´¡?ð¯¢ðZp@Åôw‹§¾?ïíYx0=¿åföyn€ç¿äìÔ	0'¿â!ÛA¯¢Å¿Ö3~݀¤*¿ïÿî,˜å?AGNbcuTXS 0151-028?ïÏ×ÏñU©?tͤE<²?F"=î}J?<¡oõtdÞ?uA)i—?tO"¿Ì~?ïÏσ‹eN?tîጷ?F4	û_
?KÅåvÔ9¼?uQ½¢¾?rŽ)ˆÃh4?ïm~~ò4¢?zàŠlq˜?]éë‹ê²x?W*~ÿp€?q'dWG®?y<C_ ®r?ïš	µ¼Z?iÆ1¯ÿÒS?Pù0Þ½5»?75çÚCÌä?‡^l¥xR«?iŽËxÝ4?ïœfL)7?€º'Lø8?]Òýíög?TXU¹?…,
5Xã'?~MB¼ß¸?ŒQ¡L?ˆ°]±Î@?Q»õQ4×Ì?]$¶ßÍË?ˆ™^>uÿ?†¿Ñ·yEÀ?îâgÞ-?F=M©±3?h";?LkE?eÑȓcëÔ? \¥Ðè
?Œt┰á?îÄzJ+Ù?‡­½#~¹?hMíRºI?Z¼¯yÑçb?¢3€Aü;?‡»2(AGN4FGL J0155.0+4433¿í´Çn$\À0Ú©÷µ®£À:b-—è¿rÀ<C8d@…"†?þ]Ã_eÁ%?Á ¨A'<°?Ós k°R@"¡ô±î@žWˆ
€?ïù$¯ñ¦¿ÓÄÐo½¿ÛÖ}»Áã¿ç2BÝË!Ò¿æ\¤¡	¥p¿Ü9G'RAGNbll3FGL J0154.9+4433GB6 J0154+4433?ì½Ö|ùм?°EyŸsæ?¢¢ì÷)?ŸÄˆrº8Ÿ?°À"ÿъ?§Öå±Hƒ?îö8ñ/¥?ŸzHXyã?‡F"'ëÄ?'Ø^fÂË¥?•p¾Ãš€?"xýEO:\?é8»[=ñÜ?°§ÐàR?¿†Mrµ»I?ª'²$ï'c?¶³×µƒ×?¢½cÕÝ?î¯/`?¿c)Ú=?E'eÆú?oøáù
ÙA?¦²F—F¶¦?{·ô˳åþ?éq‹w\?½"îNt#¶?²Ê9Ýaê?ªçò'
,t?ÂÒÑ™—?µ"Z[p;?í8Cl«Ø?²²~2ö?Ÿb$.ÕÍÊ?ªu_Ã(?¬Ê·›¹ ?¦¨ÆŠÍÕµ?扉Düx?¶ ÞÇ^€?ÇqL9z±2?±¸‹â6k?ÀDŸK›p?©P6‹BÃé?êê¦!<e·?œ
[®ë9?¢CÑÿÑ+ã?ŠtJ¿<?¿ˆåõÆHØ?–bÍ®à€AGN4FGL J0155.4-0625?ÓÉù?5dÀP`,'À:óÀƒé.,À<–'Jÿ†@r)0zò@>
í(Œç?̇œ–ú?̇DÒ»?÷¾XzëX©?ÿúa÷ì¶?ïþ\AIvl¿Þâ˜[V¿ç·y^:ÈÔ¿í¾I¡ßŽE¿ÕÀŽeˆðÕ¿ïÿ5jE8AGNbcuPMN J0155-0621?ï{Ðt9õ?ˆÄà¦:À/?ac±ör¼?aôz@Xú´?Œ§æ*Å:,?†Â¿e—?õãÛ?Œ6¯¢l?iðE"!J?uÜ2Æh?" qUÕäì?"X[øUL?îŒ]Ôw?"öÏ-8î?ˆýÛ0¿oÕ?‡G`˜š`×? ú°3.Ü?ŽnÊ*^Œù?ïP1Ÿõ?ry>ÒC]?n'šb¿*^?Xúéà—ÑŒ?'8fx…?oý…Cø²?î÷–:9$?™%ށ˜*‹?kR"ÛrŒ¤?ks%±çb?¢æ;·$ë?—¢}0ð¼?ï[Và-õ?¢Þ$™C\?y>̵K	?‹˜Ž¤4í?™¤á÷+p?›x‹®©´
?íeΉ÷vU?œ&9<8?˜²ûùÒÝ?'r–É#®?­I™bMcF?– M¨oï?íÂsY,ÛÅ?'…ÂVe?…ýÛBö?xITga?®Y'¨;ró?õa¿®CYAGN4FGL J0156.1+1502?æÆÈNÁa½ÀF€.#)À;›ªgG6öÀ<Æ´!Û@!w©úå¹Ù?úk³\¹>{?ÕT¤òé?ÊÑ(¼Œ¸¶?ööc3«þ÷@gÙ¦¤ð¿é'æ!1¨ï¿ð?ð¿ÒŠ…¼¿Ü8Ʊ•¿Þϑ7ËHhAGNbcuRX J0156.0+1502?ïahWN½Ë?®,ºaÿé?;Åßìul?8'R*kï?"cݐƒ?­ú0Ž6eÍ?ï¸Àˆ=H,?|ߏiäN	?P•™hGV?X.-¦ˆ•½?zU÷[?xx'Ï#þ[?ìşÞún=?ªñx1©–?WbŸˆ6?PϜüH½?¹uvŠoý?«ÆI€¥?ï4ï䇇&?xúû7×?A_<†Hë?2jOÑ6î?˜×08­?x åŒ›?ïzsJiI‰?'ÍmiaƒÙ?G&ª×WT?K½å§a§›?ð¿:‰?'n£uRµ?ïFKü'Çñ?'ÀC¥¼Õ˜?_ù~'kˆs?ov
v«Åû?•6è‡Xóc?ö4±)Ý?í¢yo¶$?§#Ì΂ã?\xª»æð?_ï¢1ê?·Q	Šل?§,ŸfÕO'?íôrõ"À³?—]yùXUˆ?Hª>ŒœÁ?E¯uåneâ?°+Õb.?—LúkóAAGN4FGL J0156.5+3914¿É™\]pÀ5èÍJ¡À9ÒU݂&¶À<djQ­q¾@áaKI{@wí"Ó8ø?²jËOõ?šµÉƒŸºÎ?äBÎFIm@…䀝Ÿ8?…Ñ1½¿â'Ÿ¿ùTÀ¿çÿF!!Ä¿åHùn‡Q¿ä_ÞÝpˆÿ¿æyi"ƒb¡AGNbcu3FGL J0156.3+3913MG4 J015630+3913?ïùÔÔûfá?:ç.ÇA‰??G6'Æmù?Áiºjp?DãÅ	ž­U?92[q¶ä?ïðqÚ/XU?c‡¿û£¼î?+Eˆ×Á÷?9ʆŽÏÕq?[¹¢Œ&%n?aTYû"?ïÄoÑÒ£¯?böÕ#ÓWÍ?QÚrê
¾?<pDÁ?y€`€"ñ?aÕ	Gaö?ï÷šðu:?0†Õu­8?&|³,øB??
	¨Ñ`?KõDiÑß?-ñÉ|Ý7?ïò'*~G?Uy}'ô"Ö?-U.t¼Á³? Ó¿	1®?W1†|±V?T-ª	_Äq?ïÑNpóª?~,²šÚR?7ïÂ}'?HÏXùÆg?uæؚ–Þ?}²´Ž5º?ïðÞOC?x'õ"Go?[㹜pþ?PyVQ÷¿?ˆGQ?'$%?w>P¿Sq%?ïèͼ>?Q²Ãµªø?@šÍސèz?+P'õ¾?c5ƒr£O?Oª½qWÞAGN4FGL J0156.6-1758¿íäs˜Ó÷ÀRÓo~=À;NÞÚ‹À<łw>$ÿ@Cl§s!
@EÜ@W?ÅøvHܒ¾¿«—s#¹¹?ã̤ˆàä²@9˜¸=S?ï8ßî°L¿êˆH8}õÏ¿áÊDAxpT¿ÙGőo(­¿â"^~»qܿﱺ!Ï]¡AGNbcuPMN J0156-1800?ïӛƒ²/E?emØ抈?A>BÖþ?2¤¥wî°?t
uÐÞÉ?dD~2ؓÙ?ïÊ-œU?xLJî=a=?N¤Jyó'Ì?TXøHw	?w!àH¬K‹?u¸Q+?ïlð¡›Ï?x؈nƒSM?aXÉ@`x?]âÿðäÐ?J¶Ñp?và>®6j½?麟+w8W?g.Ê`r.?IÃÜUSõ?3p>Ò<?"vüæ	ÿœ?fÒêÂ,ë?ï sõŸ?xQBô	'Q?U6?'\'?HKÖA×àp?…<t$•
¿?vς¢ÇÁ¦?ï{X
™W?V¼£Ž?XƒbFƒ^z?eˆKäí?Ž}Áߤd?©Œ<&G?îôà¨)‡ì?†˜ýŽä?lsÈ>ê–Í?fÙÁ°¬t?ÕqøE•?"y;‰Ò©ì?îÚu}-A?‡ SxFb?cÕ÷kÐiU?UrZ–ó?¡N±†"Ù?‡8¶åÕAGN4FGL J0156.8-4744?ánšÊ=½ÀPp@ ÇÀ:mDù.T§À<ªfÄZ7"@ŠÃvˆr@Õ~œ¾H?¸´XaÀå8¿›ûÚ'ö7?âa0œýç@	i°|ʬ¿è6úhŠ'¿ãe—=$¿æ
5bhß¿Ý2GZ²~¿Ýw¼Ú¼N¥¿êNHÝêVvAGNbll3FGL J0156.9-47422MASS J01564603-4744174?ïøæU¤?<j•Ú|ç?&±b+fJ?HÀ¼ãP¼?H"‡"¨?8´'xÿƒ?ïïÌuÜG‹?b?Ä,h?)H¹ù÷Й?9¼hPNù?]=üï»}?`Í0!ÁRê?ïÄäp#öÍ?kš'ŽwÅf?M;와n?5ÑÜ.?£?yæeä:?k!öc¸ÐÛ?ïï¹íˆ?e?A`aðÁ ?*b¤d_k?çm•á¿W?]?ÐHW½?@ÆC™?ïðh³GÀ‰?Rò]ÿ/b©?9Œ¼ˈ§?,<à:Ò¶´?XËiáHA|?Pëç(ÊwÔ?ïÇÊ埊'?€ËãF¢'ø?>|~üYИ?S&­"ÁUµ?z2Å9ÜuÜ?_½'·?Ü5?uè%i®0á?W±DgÚK
?`©¿­­?…`àT8óY?ss£Éëj?ïԁ=F ?`0jö×Ùä?B÷LT¥ÊY?2Ì:ùÑU?sÕïÝ\`?^äÎ[Ð-ÓAGN4FGL J0156.9-5301?ëqÙX˜¿ÌÀN°å^³À9Ü¡|¼êÀ<³†ª©Œ@¡ 47?øת@°Ê8?´->§…–?º¶¢Êê@F"Ú8+@‰qü­Æ¿ïáâ"Ÿg9?í…ʬk-?¥G´t'Ln¿ÖŠš"U•¿â3EaÞí6¿ÂèÛùe‡AGNbll3FGL J0157.0-53011RXS J015658.6-530208?ïûfì£Ø?3.Jâ'<Â?®Ÿ
º´…?£qÌj??¤0]ó™
?1j@ªŠ?ïsêf?f_:—?/'çoϔ}?Cxý¼á¡¶?^â­í¸!"?c™öé-d?·ÝQ?"<]©Suô?SrO;?A´
žVî?‰qÎ@À:?"g?kY!?ïÁÏy‹˜`?a«ªñ	\ë?8.šÁ¢2?" 
峩)?}–ðeŽë7?a>/‡úWA?ï÷ëù°'?B	m1ƒW¸?%̺¾ï$©?JÙa£d?JÜêŒ[Y¡?@¢>Ûô?ïǎJ—9(?'3"?MЅÓð§?~b)`-	?x~Ê
'SA?…$Ü/»"?ïO îY~?
¥Q€½?cQǖ¬¨3?h±X?"¡µVjn)?‹ï®_;?ï–<ù
P(?t=}¢ŒÄ?A6Ÿè™D˜?5×8 4@?‰]WÏÚö?sܬ¾%šAGN4FGL J0156.9+4648¿éua‡ô‡À--"n)ÔÀ:ë<©Ôz@À<h-æÃ@Ÿñ‹¡´?ÿ–îú>¯?Ðy<¬Ù'?՞9¾g¯@Xä1ò@þíï]'?ìç`vã6?ï­Ù¢H>Þ¿Öl|ªöc¿çˆD§Ï½B¿âtÒ9ô¿ðAGNbcuMG4 J015651+4648?ïs®à 
Ä?'ö¥QË\/?g¼
Œ¬é?b,š¦«™*?%GäÐa?€[г%x?ïiœþ˜?''™'Z,"?p°íq%½Å?}®ó"ÒÉ?@:Ø7?Œ¦¶šp]?îé&…áçø?ÆßPq­M?‡	o'e?ƒ¥¶-'‡?—V ¸¬5Q?….…×ùYP?î:¾"'æ?"²bd5?Sw`¬Ð?sNcz¢­D?¤ÿ8Ú¼úr?€À@Œ_?ï&@INÜ?‹ö;\ׯD?vÕÔÖI?jYd·Cƒ?•³Á––b‹?ˆÀYM®qˆ?îsnXÙ?®ožŒ\?'?Š"=ɖ
?œ?Ýü™?¢Bµmp×ë?¨X¸¡ô;?î4÷Y×ü?–¦¹)ç6?'<ßjšcÕ?ŠÞ3ø6$X?¤! Õñ5M?W¿œ?ìðÍnC'?šâÃ5¸
?˜I‰§WI?†»1d"
Å?¹Ž+"ø2?—SÞ·KAGN4FGL J0157.7-4614¿ì.ç|¯ÀP´˜5‹'À:LvѵÀ<!4x­Ç@ˆW+µæV@ê}ík¨Æ?¿à	ëf?û?ÌꗸîÉw@–l£—I]@A	—ÙP?ïü=¿ÿ	¿Û==ÛWÕ¿åÒ¾^"¿èÛ¾WîÔ¿íþ˜ ó–¿ïÿþR€ÖTAGNfsrq3FGL J0157.9-4615PMN J0157-4614?ﮏ?MÃ?uà42Ër?r±4›Ð?i³F0>u×?v,KbÖñ?i ®L©?ï⊤3P?p‡|œm?:'0ŒÀ*?DðBkl?j#5Çߓ~?l‡ÿ`nî?îí™ó‹¥?'¾!m ÝÕ?Ñ½ºo®ã?‡gOàâL?"c⹯Ië?ˆ@"'2?ï·ŠLʉ?_ÂN¯""Š?L¿ ĎÕ?44"…:?€q+mïU9?]§Ä 'm?ïpfèÊâÅ?†èĆ–?iÜ	"5?|»<ÆH¾?'|iÄÕ¥?z6ƒÚ~0?ï¦0ŽÆµd?ŠÖæä͊è?RŸ‹4Ûb?dÂdÑ×FÐ?"êë>§"?‡"ªÈ`Äu?íø_F?œå3h:»Ž?œ5	¶²æ?"@Ý
Ÿ¥©?¢\¥-²¦í?"ö#‹´úT?ï2†&9Œ?RœÎŽ8?c&̛·?RаË|"5?—Ja­W=?}V%Ì¥AGN4FGL J0158.5-3932?Õá uù"ãÀQÕQ֌i/À9‰'TPº-À<L~D©}<@îJ µ'-@LQj‹?®p®hß?®¬ˆ×[@Gjdø¨@ÝÍM{2ü?íŽ:‹I¿Ý—Ä{Dš¿áž¾fØ|-¿ãâC çU¿á^û}å3 ¿âaÈýŠYáAGNbll3FGL J0158.6-3931PMN J0158-3932?ïñë¼É?K,•Š.È©?(0Rèz°?9t¹^¿ö?Y#óÆ|ùÀ?Iµ¢¬i?ïìó•°Î6?h&ÞhO?2ØÌ3(??A*¬Æÿð?`ÊÏ:ž*?dùóóî~í?ï·g~yû?x^úma/Ú?]3"gœ?kú|%µ?|ÿ¶ù5¿_?s/á•>ê™?ïÛº7?L
<%Å?D™3YR
Š?)܋îl(?o¯#jҀ?JR ÙC"Ï?ïã~ÅWãl?a4•{ÚCf?;žé"íÄ9?2̛på?i
]‹ùT_?`v9ž®k?ï¿>wgž'?³0 àœw?F"8V"Nƒ?U;x°ü›Ì?}œ}'1Âý?€W*·éX?ï‹Ê&"E?£GƒÿSà?aÃR¡tƲ?nÃ2DJݟ?ˆœ©Ìö?~Ì«~ÆG?ï©»"â?k'Nâ\õ-?WË£>p?Dèöœo?'ÁœÈÆ(~?i(ªQKnãAGN4FGL J0158.8+0101?±=^O«ÀLÁ¥~ª*À:MŒuĨ;À<W#I±$@.û%OÅ»@d¤Ú¦?µ3>ñ­V濱*óÄa?úõ³;?ï™"/¢&}¿ã·M>w4¿ßêvjG¿éI­=ef6¿âò|Ÿ7é%¿áa¢
×I¿èËRä©bdAGNfsrq3FGL J0158.6+0102GB6 J0158+0101?íìfÓý Z?Åȓ¨Ïþ—?§ösþ;¨?Åçù"
?'†='}¯i?ª×"6ڐ?ï<D¯ºö¿?¢Z<é¦?z4«i3úö?†ˆÓÉwJ?'ê?1?Ô\? >¼R|Ð?îk*ÍLé,?™]׶/³i?‹¤ŠŒ¬
t? Êá÷<ž?¢d0Ššæ?'"ÆH°:H?î ˆ²QÝ?ˆ¦'Ó=;?'1`ã)7?tøæö4 T?¦"(€ñÌ?"§:€ª@x?íÌÃ*ó¯Ì?µ–•zw?šKñ¾Ž"?²H
,jq?¦
Ԅö 8?¥`;ÁwØ?í퐼¦9?³ÚeÞ…Œ?'F%'$¤&?¨ÌÚý·W?¨ál.5ú?©E¦ÝŒÔ?íu+Š6>?nY ™ã?"ó¿à?l?Žœ©^³k?®³go&³±?™aL¦?Òû?ê©OÛ¤E?¦ŠÍ.3©'?§ŒV0—?—Ma'þ5I?¾ñU±Ò?¢³Ëü›±AGN4FGL J0159.3-4523?è˜WèÒÅhÀPÒt>–=ÅÀ;ûAT^&À<ZÁ#>@ƒ+̱º@ñÀoz?ÃïÊhC‹E¿­Ähœ˜ôÐ?çM}å-@
·y
²ñ?ïÆ­czù›¿ëϚ!~ÕÉ¿ââ΁WÙ[¿æÿ¢!¨qN¿á¬Yûð¿ïÿýç!éAGNbcuPMN J0159-4515?ïôԏ}¥·?xws†ŒÚð?'sípÁzÅ?Qåëy†
?Shcp,­Ç?t
(ÈU)·?ïÚcÁÍ?s|~ýË@/?A𾹬më?Pby#"ÍÛ?p¸¶5Í¿€?pxb·
:è?ïPûø€Ò?}ñÍ?^¢"U¸å?m²lKtœ?"÷†ÀÁ)??ŒÞaéŒÈ'?ïáiêÝ?OÊD›Ú‡?+êèpBÍ?£/¨¼n?lå'M˜aÓ?N°žÕ¿ˆ}?ïíB¯ì±?b4èhTjJ?2frڔ¬?1þ¬RÉU ?`pð€?`ô}ìÆš?ï¦bZƨ¤?‰Œƒµ¦?Lññò¢6??`P*!Ø$?"˜J·IN?‡÷mO?îÎ^…ˆG?–Rœ/ )?ižãe)¢S?sá4r¬O"?¡€)tÝ;t?••ß6´?3‰ð.?qHS<#X?F¾Aµ
Ó?;0Yý]÷u?‡ðŽþa?pӛñ'=
AGN4FGL J0159.5+1046¿Ý"ÃM¿réÀHSπÜ3rÀ99I—"ÇÀ;ù'ì®@¹O"ðB?ÿa,:=é?­ÊÞW†? ¥ ÛN½?ó(᠙h@Aàz~¡F¿ÝèÀž@Gn¿Ý/ò6ᄿà†=~搿áüŽ''Û¿Úª-e"؏¿ÛLáD¨ücAGNbll3FGL J0159.4+1046RX J0159.5+1047?ïñðr
ä?OºÚaêv(?)Yoë!·Ã?sž€|ëó?Xô²ú}±õ?MVl`É{"?ïæ'ÁÁ´s?kH[–°,l?3hrVN?AÌ¡ïs–?g0
!CL?h8µo`O"?ﳔ\¡ä?nukg±,ò?SåÖÔ¥˜²?@p¢ßq—ü?€žB@"d?mt[MÙÔª?ï±¥ñãÿç?`Œ‡ø•?D©X)ü~)?)É*T?'Kíößa!?_ô'œâ?ïßEFuô?f:²@u	C?=tæìYÖ?1ŸÁÔQðÁ?m6F	?d'cõá¢?יּҧµÅ?"×16ð?A–4YF¨?Qó
õ}B?ƒ¸(	8TÝ?",= G|L?ïDÃJå?'i¦™%».?YÌgŠpa?Q{
ï'0~?•D£²?ÏØe÷F™?ïA¸!"?|]—:y2?X'±ÿΣ-?Ey³FæÃN?–Uýá¸Y]?{Ê)ã3AGN4FGL J0159.7-2740?áÌÔã¹pÀRµ;Ÿ_À:"z-ëÀ<ÍÄC'O@È÷C«@
¨_/:€?·iŸUñ#?±]CRAf?÷Ê	ÞÒ@È7Zµ-I?ï÷"_mλ¿Ú]&š¯™¿àÁÞây|¿àÂÞZ"Ê¿ââ½ÏÚ¿æÑT¼÷"AGNbll3FGL J0159.8-2741PMN J0159-2739?ïÓÀ*
Uå?`žS‰I?GßÕ9ˆ?8L ÁlÓ?s#ðmŽjf?]Yq‹ µ?ïԘވ¶ó?sÊa|`'?GGß^(Ý?QݪwÍ8?rʔËÂùG?pì@Žw¦?ï€A–£E?qÄkèy=?cŒúnúÊ?`
6…!Ž?‹[»ºA?nz	¾À#­?ï"qëº?b.lΧ?d^Ò<-?Eµ™F€?†7šúVn?`Ž«{¶?צּ-J2?mcD9!?YY\DPö=?H+ 8֕¯?sMûñˆ…?j'œ¤ŒÎò?ï'é=é?Ž3ª`î?[G¬EÿwÊ?g&cNė?‹ÜºüKݧ?‹~"ƒÕã?ïOoSõË?ƒïÇ!ì?pçhyÒ'?k"?_H?˜¼7öˆÕI?€×CÝË-Ù?îû:•A	$?|²q£!ªå?wRˆq?bGÖ8rk?šÄXêI?yßsÞîEAGN4FGL J0200.3-4109¿Í3\è}MÀQ"Ó0"'À:‡4–àµÀ<'oQÇrñ@ p6åDgä?úéQgÑ q?ÁblÇ(ž?Áۛǜ6W@)ý¢W®=?õA÷˜(«¿ïÌ7Z?åéáæ9…]?£ûüÞпښr¦æ‰¿ßGH~sùL¿âÒ*AGNbll3FGL J0200.3-41081RXS J020021.0-410936?ï¸|ŽI?sßnSÍ4?OPU¨Ø?Eû׏9›?јM'×?s…›Gˆ?ïrL¹6£?"L'iÆ%?r¤¡Kïá?~âLJbM?ŠN?‹–í×YNÃ?ïE¤fž'ó?ˆ]ãúªšb?n#(.?qú6'Í$?"‡!ŒßÐ?…–lj@Îm?ììåގÀ?'-†ç?Œ©†À†¿ä?r7°ç9=?µ 2¢Û?Ž «£à®ý?ïv|4È£a?‡4~,Ö?g†¤ø±ýË?aUhÂU2^?ŒI‡¢M?…'= ð?îžÝ"f<Ü?¥Õ(½˜º<?‡
õñ$?'(9Â? Oju…6?ŸºÀŠé
m?îÒ×e­?'D÷ŋõ?tûp«D'?t­e×´Ø? 3(ºH
½?A42*Ø?éÓ	ó|l–?¤\Ä©¢,9?—JbD…Ðk?…MÓdÄåH?ÅʋêYz›?£•'ð¡†AGN4FGL J0200.6-6637¿í¥Mܤ'´ÀHŠÎóÀ:#8ê,YÀ<…6žË2@@zž×œ	@ÐeÁ•?³î`¬ßX?'dmÆ_¨æ?ÙiôE6ÀÜ@pXËô
¿ám‹zÖ¿ä'z¡†Î¿çúVÞ3&ž¿äUûŸž¿é±Èd¿ïú3¢Ä»†AGNfsrq3FGL J0200.9-6635PMN J0201-6638?ïöðyû»?D?"	_q\?,nP€€â©?"R¯¤U?M"ƒ³*"å?B5O †S³?ïèî¿ÌðD?i|÷"õi?1X,¹nu4?@1I
½¼?dæ:ڍÿÙ?füÈÄÓ¤Å?ïºOÞ©\õ?rFúýð?SŽsôåå?A4Ïò?}ôsÆ%‡²?q†SmÇ¢ü?ïó®þ'/;?9Ø¢ê`g?4r-þß?g¸p˺ý?S ¦Ö$ƒ¨?6ð'!Mt?ïèŠuN<?\nch»ž??°Lú\?0‡¼œ`}?c€ßP—y?ZÁw'áT%?ï²á¦p'?…B1£Ü?C"ïstÁ?TÇUõã×?'Wzým?ƒó™è?ùPäI?}þz&´5+?`ý ý?V¦¢/Üè?Š'Úi–½3?|Ëņ'D?ïÝxÖf»?]O¥)þª¸?P6¾x'?@7¡w¡†ª?jÝ}ݛ
!?XÔ¿º‰ŒAGN4FGL J0201.1+0036?ïr݊+´ÜÀLÌڐî¢À;~eæä¦À<ÆCnÙÒ@!4՞'?ý4¥ùú-?Ñ"×ü?®-žÁ0?ßŐÃ\5¶@‹ìé͹‡¿ïL³'#i?ít來
 ?ÞF}¯y¿Øá<O¼¿Ýü"C¿‹¿àqS>ìNóAGNbllMS 0158.5+0019?ïô}Õ»*Z?CÄïór!¾?P7/e³Ÿ?IýÛ¾)?U_P¤[Š,?C.¼ŒPñ?ïäGe_M?oˏU^~?3~Ùp€ÖL?A,Ö°C'?iH¿ööM?lîJr(_D?X"ý?n·r"×M^?X:ÑҎ	p?AaÀP·FÒ?Š›¸œ?m¯¿,œ‡?ï§by5º¼?f2þé
X?Cñôº0?1¹¬ãø1?"èB_{.­?e¤7:Õm?ïì˜R­Þ?RJ½¥©Ó'?(‰å½*/?7úVhÒ?aßüÆQ?Q‹R 3+D?ï¬Qb{Ó¿?"Õ±Æã´?K6¯þPl?`¢Ï —?ƒ8<xQƒ?'š¥Fñ¸?ïE_±§""?~_S>0Þ?_!4ÅHc?Rs›·
؞?•aøÆåR?|°ŸÑ‰M†?ï>3J,?`q‰¢$?N'²ˆ¥%‡?GоÉæbb?—Eÿ|wu?D¢mAGN4FGL J0201.1-4347¿î—šë)ÀQóà7ÝÀ;­†)zLÍÀ<ïÈN¸Ê·@!ñҕ¹?úÞ@'—?ÑV€[¯ÿ?ÇZHJòlš?÷žçf¬"@4•¥RÝ?âÖtì;'?ÎR	!¼¾7?åǂ«@‹¿ãæxw¿¥™ÑÞë™}¿å²?'ÌÎAGNbcuGALEXASC J020110.83-434654.8?ïÎe³ãò®?f$i1?G&‹°•½?8bòôjÔÂ?uèT›@k^?d§/	§üb?ïƞ?Ï+?ï ø¹Ê?Qí[G~?_ ©S"
?x5‰Gé'ù?yí‡õ-Ç??ï9h¤Y;0?"D'nZ?cÐsÔò¸Õ?cÌn
NM?–XÜú'8ï?ƒѳ|Ý?ï`
WOzÅ?vf5L릏?@phÂ?5á6†Iv?"~ŒÈÕæ?uõì×lE?ïAאË?||R"€Ö?_)],½	?T[7y­°?ˆÌDë9m?zy¾‹˜Á?ïza—Î
?g£Œ¾h&?V¸¼ÚœZH?d7'3H c?Ž¡ü©.C?Ž/ãÏF'? }t±?'tOM—?nš÷Zœ†?pž¦Ã?¤fƒœÌ?JÝ趴É?îB˜€a[²?"²­°µ'ˆ?Iì«jçïÊ?G®uÅsÔ?«nÅKøF»?"'»ð)ÊßAGN4FGL J0202.4+0849?ïvOÖ4³ÀI0ߛÜjÀ:Ðè¨ËeÄÀ<tíSUª@ õ.vŠö¿?ú'4Û©ß?ËÏö¸X¡'?̸Ž;íkÿ@H&	@Êúmnî?é¥C†g®¿êâàíB¿º¤›?áíE¿Êü¬äOx¿Þ1¯$›?â¿çJ¼¤¡5AGNfsrq3FGL J0202.3+0851TXS 0159+085?ïÜé¸?÷è?`xmŒŽÛÞ?<YòM€q?C|Œ]N)?o‹'[N³T?^D­yv?ﱩ¶">?z.±9b"?T¢k7ˏ?W'€¾ v?uí‹<î?v¬Ò"e`?ïhl· æ?v5IJF?aEL?:ª?R…åÑæE$?Ð m¨Œí?tü,;Z?î­F™0Vú?}i¼±Ê†'?cbcÏi©w?G/"Κ?£õp,~\S?|Þ¢ï›n?ﴞòì=£?vrn£Ð?JÏ&ŸAh"?=å–ílø›?+Pâ*âï?u˜8
Ôj?ï?W:ÆÇÇ?"x*'6[?bö˜ò+‹\?mþmˋâR?•¶Eœ´›?']¦©k€?îÚÐÁŒZ?ŠvU»¬©?g»^y«½1?cŒ{c¤›P? Øö1?‰VÒ-­å?ìzl'ÐQ½?—ÌÒPü9$?s¬£|fkæ?b´UjGW?ºñÑ1>?— ˜ºÂ AGN4FGL J0202.6-0258¿áâïÅ0‡nÀN9a€M˜9À:sëLÔÉÀ<cݯs²@7súž@óI¾ó(?¿L͹ð…?œÒ¡^E@ã?ÜðqA¶®¨@À¿aKæ?ïóÒà¿ç1e}³4¿ä͇§ÿê¿Þ¹%˜b¿ïÿÍ?¹Ss?ïøŸƒ¾fAGNfsrqWISE J020239.94-030207.9?ï]u67õe?¡)Þj–è3?sñ8¢œ£?ƒ«V)]>›?ŽªdQ€?™ÖËÈ"À‹?ï¶Qu¾s?€:ù°ûÌ?Xt×OØ…?^o¯6?~ºD'`'?{9ÕÈÁO?ï mOR'c?ŠuÉvO>a?}²Ô–Ù?‰?€/ō6ãƒ?"… êûôÉ?"j9ęºã?ï‰ø–¡Žþ?jñ6F€?aۖéH6?H¤SÉf­?‰
ôà,g?h\¿»Å¨?îËEUʌ×?™‰åtq>?……@ò
¤?€A࿯Ã&?›Ô´Å8?–9&n'¹?ï?椱?™‰"}Ǐ?h·	‹«ÚŽ?uëéìññý?"ìJ=&VJ?•ØÀÞÈpô?}Jê›?'˜SæŠx?…j4èo3¢?"GNUö1?¡ÙÚñ5‰e?Œ~îyn ²?îy\Âpî?Œ.õ×u+Ø?K‰R9×?o5ÃaÖ?¤€Â­Ã?‰9Z'éAGN4FGL J0202.7+4204?År"‰d9³À2ÞD""N×À:¿í½qæÀ<ŠÊ'_éu@ŸøUӍ@ª‰žyÓ+?ÅJ¢Ô€Ë?·ßT"@X?òΝ‡dä@M>ê¡t¿éæÓ^6l#?îß¦Ä$ˆ¿ædèÕ.›¿ØÚf}ãZ®¿å¨Ñl×Å¿ïþÖj€˜AGNbll3FGL J0202.5+4206B3 0159+418?ï÷·µAŠ?83ß7eˆ?þ=ò"?	"§'1‰?M½*÷Re(?6v± tu˜?ïìò«ûœ?fÙÔ奁É?-ƚ¯|5_?<W¯ôöXf?a0ërcъ?dg£hª'X?ïÄmSj‹?f·ã°×½?Q3àø·ç?T`1ötŸe?y¤؍,q?c ÜOëàl?ïÔU)@?Pbôu?¬?P	6"—´k?0©ZœnÜ]?qÓ$äh°P?N5ŠyM/·?ïñ·ý ÁZ?J­³?a>A?(‡Ã…'†Ñ?wì=&.'?Y
8ç?IÒۇH?ïÆÙjŒ]=?G÷ÊÙ*õ?A¸<üØa?ReÎ6"q©?z\Cb± ?€3$UƒïÖ?ï¥?幘?p>üb7<ã?V˖³_D?U¿ð`ô¹/?ƒÖ"è…0?l˜Ï(vˆŸ?ŒGvŒ?k/@‹¾–%?b	Éq?LÞßõj?…
Ûÿ¨hÖ?ht£ˆAGN4FGL J0202.9-0225¿ì/¾µ)dÀM÷Õ<ÝÖàÀ:Ó¡ÏɏÀ<|%ä–.@ ÈAÒt>?þŒÇÄOOÉ?ÄÊàä[ߥ?AB g"×?þp'Ldë¿ïïê^-1ç?ïá¢!¨¿à:r•;¿Û907Ö0#¿ê—Š@
\$?ÙTÎäT'õAGNbcu3FGL J0203.1-0227RX J0202.9-0223?ïö¼ú
·?‡"Ùø$ñ?Rm4Ä'k»?]òE|ê¯?†4ª!i@½?"? ¶ºÆ?ïÉÕ¯}Q?x'àc"¼F?NÓ _L­M?UËÎÇ7/l?w:´!&`¨?tëTƒW;e?ïc
z!?ŽIH¯'uL?s"B"Æõ¹?xôÓ)DáH?—RŽ7þ®x?‰Ùq"µ©?îÝrw]–?€¡O:Ž½ç?pIë<C?VɊë.v[? µ‹"R›?Ÿpì?ïkÃ`Έ?‰5ä›ÿ?`µv"?º?XA
ÁՒ	?påÜÝ?‡m©"d1?ïio,³'>?'è!·ÁÀ?`6ú<ÅvÎ?jLˆÌDJ?Ë;±he?_V
ª?î€õkQ‡²?–£ºNÌÀ?z%ÊÆ'ï?~kTã½Å?¤«ïï}%?"»»Džœa?í V¨"ot?™'Hl¡%?9îÏ.8'?r¼9͛?´Öák¾‹?˜®R«¡îAGN4FGL J0203.6+7233¿ìÈ@">Á@$ä$=Ìê)À9ÛtÄÍúÊÀ;Ü|©žÊ[@iŠ·( ³@@Tƒæ?½Û"zÿ$¹?¬`áZàK?ðô:æ…Û@0aV݁?íh"ÿ‰;¿ØŒö=^…F¿ã¸j¤ ¿ã¼]ž–®ƒ¿á…òB}(¿èRçcQ0AGNbll3FGL J0204.0+7234S5 0159+723?ïgÁq5?¨©•~ñ'l?I¿ZD¿ë)?PmÂÕïâ"?'On%Ø?¨"µÍÆ?îÌcÎå‹?¦GB†N?]ï‹?cÈPÁ¯|v?¢M³—:§m?¥wŽ×É«?ïSlŽž"?ŒÙWÚ
{^?jü$Fçá?e…€ZGçþ?šv
âçwe?‹§á"4š¡?¢ïâ.?{7†ï
å?p'd`Ž k?L;UªTý?£yEáíŽ?zâû±'[?ïuÑ»žý?•Ø€'M?XÒ<Y?M›ËtÁ—?‰ÍH‰?•¨mnƒÆh?íH®Hc'B?¶‰Þ'2?ps/sÊJç?à¸6õ®?´³ZÆ+:D?µèâêáÙÑ?îWŠË»?›—"iÒC¿?y,2'5t9?tý|¢
?«Õ\@?šºÉƒ?ì©õK4ö?˜Ý!ydb?ˆÚo͘NÁ?pZl)>RÏ?¼Ïb[óNt?˜ímΦAGN4FGL J0203.7+3042¿êòPW0h~À=£gŽÀ8—'¡}"À;°-,ˆõ@z<c3@ )»»,'?£N O´Q?¹9@}ôwŒ@¹Wɱ@š³ÿʥ¹ãf_¿Ý¶µÅIK¿ã½ÊÁ.Þæ¿ââ!LÖÈ¿éy"ù÷¨¿è²#3
ïGAGNbll3FGL J0203.6+3043NVSS J020344+304238?ïÃÍ?–÷[?¬"¼"(ŽØ?QCàM´É?D¶~˜‹Æ£?yÈh@›Ù?¬‹W·V?ïçÝ÷cñŽ?hþ8x*Y?2õx—ûª	?D9h1×p?eÃY¤h¬ö?fd=ÑƆ?ïºÁZ[sÍ?wêNéÎ4‰?c>YßØ{?q1Œ¨Á?y%ÿ•åA?pEm½[·T?ïð—/˜?BÄjP5ÒÚ?%"I¼³Êæ?0{$	?],H™?A¸P'7A?ï›í8ýøi?‡E+ø@¡?`9ß­v±'?W©bîA{?"ö9Ólkg?†åðmÞ!?ï¶ü€Ÿ?""Cx¸"ÿ?PýeÝÉ?hÔß90€?€\"UŒúO?ƒ<°†W^í?ïŒçÖ#ÉÅ?††4}";ï?tÌÀpD¢?€ßçìkÙ,?'¾¤\®k?|GzùÙ;?ïփy"
?ažã{'"5?;«G«œ¬R?0)à>XC?sŽÛõ'—?`›_˜r!bAGN4FGL J0204.0-3334?â-}5N°+ÀREQ.ƼèÀ;1ºÌð;À<Ïïå։@ ŽÙw*.?û­ L;Aõ?Ó5šìð{?Á61u?ðßn	È֞@Œ_Ó¥."?ïK°¢ÊšÃ¿é÷3þŠ4!¿×c.qÊH¿Öž*¢ëÒÌ¿à$>adŸ¿èý?[_¢AGNbll1RXS J020413.6-333345?ïÌþ˜CP?ÀëƒWtc?› âáò¿?Àõ
Õ,S?b+íéª.?P?	‰ ?ïÖ¡gÌË~?t*L©¼)?EdñÖØ*?R|¸SÒ?r
_\,‹Ú?q"èQÎ*?ï€òEy©1?q—£XµÒÎ?W°nÙ*?A¶´Ìo…?ŒÍkxáøŠ?pârM¿ÄX?ïŸèÑmÎî?b¿8J?BöŶ§˜j?)	t¨ˆqÁ?†Ö_K(Ã$?aÍÏÓro?ï	–gò?¯z{NÞh?†
'jY
ƒ?¯‰­ðìü=?s`æ
'«k?cU5‹Xv?7Sä?‡åérW²Û?QÂŤœÒh?_›0'O!>?‡Ýh_N•?†jö­PC?ï)â#mÈ?U§Ë
RÞ?_ÊLM¹+è?WD ÃPk?˜ÇǛO?~G˲k?ïÎÁÞK?~.˜)¼â?M-ºô¾þ?A
r
ÅnÒ?œ¿`J?}àÁù»¯AGN4FGL J0204.1-2919?Öð[å%€ÀRuæFñVÀ;«*ÏÀÀ<÷P²ŸúÝ@¾žÆ)D?ôÎ3Ÿi½3?âUÝLvÑ?èõ €"Ž@V–8@[ul=ÀÖ¿ÒÞÎWˆ?åõ•äsx¿B­­ê‰v¿Ô1‰$i¢¿ç©$@üõ_¿ïü5ĊßAGNbcuPMN J0204-2923?ïÆOá?ƒ§°Î??R°6¼œ'd?JU€é^"×?x,kÍ^3?'ì
_Ádñ?ï²p+Gg¯?‡Aêö4x?]‡EbÄs?i¸Yž
?f›Ó?ƒHË]ÒgB?ï jŒCxX?Ž7*j‹?yþ*á׫5?{õ¾†Ù?•s#Ãf!?‡‹
ý¸f´?ï	>,¶lc?{­X@P?gPü»]©Ë?U¢Ž<È£?›îØÑñW?{FBÊùå"?ï–ÿÖýè?Å-x—Œ?iàÉ/I?i&à°Tª%?ƒÈ"úÓ?Ð¤Æ\?ï+'d}b?¦«)–?tÙñ«Ù?"µlÄâ8?•WWɎA?žŸPÍ(æt?î'wôÙ0]?™+†›âŠ?}¢b1¢¶?}´%3²´D?£FldÆíÔ?–§ÇVV¨ø?î8‹4¸*?'
ÿ|_g"?cͱäÀ?d·pä«{?«NztUá`?'µ…žÀAGN4FGL J0204.3-3140?æIfÑEWxÀRa	éÍ³À;nÈÏJ«À<á4s¥J@&ky˞@d‰Ø[?ÈÐæ¿'æÜjl?ÊîVŠPPz@˽€~•‡¿èòÁS¿ØÔ¹*X™¿å!s¸^€¿¿ä´_î}!¿Îüâ~ºÆ¿å2R˜SH|AGNbcuMRSS 414-035156?ïоsÔÊ?e»B¯$·Å?:2B¡ù"X?'ޛ¶Kà?vPüš	sú?e먈2?ïÖVMênž?tEЬ?D'[I"\\?RßÄ:Êß?rOí˜ê0,?q¨²lË?ïa"•^Õ?|ƑËú&é?`ý{òcè?W;R&îuL?'»ýÐ-ˆ?|ÜU–ãn?ïÒF+æì;?W¯Ð,ø?1ÝÍ-A<?=ÓKGKK?u¿
I§,l?Wž‹ÒÎÇã?z	í{?|h€ò)ºÑ?J³qR'*?9_Òw'?‰¥*tÝGz?{·ÆÕž*?ï—O`vž~?Šöô
àè?R Í»lJª?a4cÖYi?‡è<pÙ
?ˆ–ôFå÷Ô?îäµX´C‹?‹Ñ$$–p?gLä YÉk?bo¹-0? ?Ü2ø#2?ŠX+äUÂ?ïmjiÞɂ?zŒàCd=?H³ñÊ3E¢?B,€œTЃ?'8ôŒ?yÊ3K!2 AGN4FGL J0204.3+2417?à{YïrÀAÔdE#öÀ;8é
55À<¦²ò03¤@ ãóÏ/?ù)p;Ò>&?×µZÀ?ö?Ô
ª]·U?ÿ"!bPW@®A·/£?ïÎ3i¹×þ¿ÒÙxÛ^¿æ†00Is翶Ҫ¡¬¿Ñ¢#ᆘ5¿ïÿ® A§AGNbll3FGL J0204.2+2420B2 0201+24?ï¶KìgœÇ?€
Ü3Š'Ž?Iý3¤Þ0?F‹Ü´šøÊ?€Í1¨ÄÜË?~"癬?ï¼Á]Ç ,?}\sCO¨7?NVœy?Yª&à	¯?}Üh´PR?yȍ^‹R?ï(ê™?Ó²×ô—C?hÉI%‰
?q"C'¾?—ú©"‡'Î?Ž
ªOŠ±é?ïtÓÛ£™?pÝIV"?Hâ8r&\?8uÊ'ásÑ?žsݘ-%?o¥¢3?¡A?ïWß$9¾?'"­BP¯?ZÍAÃðo?T'K<ùÓ?"WK¼"!ì?c粶‰?ïSœ	òƒ?'ÛäL-E­?^¢ÈLv"x?ráƒgÑê?"²ÿ÷:—R?ñöÚL>?îrÕo³—?˜ž#ÑrL?gZ	þßÙ?p;Híbü?§]b²Ï6?—¤QVÕfß?îwPÖ©'×?"`bÆg¼?XDÒs$å?T֐ƒþÐ?§ÈÌã¿^?")dl*AGN4FGL J0204.8+1513¿î¯ºç¶ÌÊÀFŸÂ¨†œÀ9Q/¯ðóôÀ<0rÅð9¹@Œe¨%x‹@ª?Ú
£?­ÚÉ呿±?µ=+Y m@ä¢üïªG@ûû˒æ?~Ãvˆr€¿ä"¢A]îH¿ã(Ÿ[zz¿är_îÓ¿êl5恿ïüÑaÜéÐAGNbcu3FGL J0205.0+15104C +15.05?ïëîk,€?Rh3ãŒÍÈ?7þV©¶Ø?(¾IŽ:cº?aÉýtÀ]?P«ÐùŽ>?ï×xþ!69?v†a±Ž?DYcåc?R»Ã}'Nø?qÀ•¼×?¤?rúJ
?i?ï®5y3ž?wÝ4vq‰?cæfšÌq?o–‡ë@0??	²þ¸™?qbLû')'?ïâ2s+?LÂ#±«Ö?G8O*²Ý$?-™«$¯Ï?gÿxÖ^{ ?I¦â]?ï׊]'€›?b-Ç™?Kd¾_«ãj??7¨s5?pÎ9Q	þÌ?`'ü€5óÁ?¾ÿÑÿ?‡Îö.FÅ?Q4^ W?c5H¶TG?…ê"q(:?…a_›öª?ïn'H'È,?…å¾q{~?r4"#‹)z?w²),
S?‹A+ÜaF??~¡5û%®ó?ï³Úÿo%?m
$Ÿ†=}?_FÖÌ%˜ ?M©kˆ*Nà?~A=«'Û†?hšK8?9	AGN4FGL J0205.0-1700¿éêwwÛ®½ÀQŒí"1{À8ôh§‰FeÀ<DÕòæ<@Ò}'Þ[@ƒ&ùz«?¨x'¼›?´ç<t$•@XxœÉÏÂ@Ôo{bø¿×¬| 9›Ø¿ä¸MžïCð¿èpžmhä¿éŠÃæ¿ïýò߆õ¿ì"ñÉÜW"AGNfsrq3FGL J0205.2-1700PKS 0202-17?ïûNµš¬?2
µxüR?!ø6Gѯ?ý‰H©˜§?<¨w9C‰?/K´>á Ú?ïä
CÙQH?rzœèÔKd?>Q%ús?WQ,E•ÏÍ?h+—¡/"º?m¾HÑ°Ú?ï±LZÃèD?}ÁšÄXáK?aBÿ#Ï!˜?l®Š^Á–?~¸S$M(?xZi¥WŠM?ïöýÇZ`ã?57
Ž·ß?1ºµV
?ԛïF®å?K…)­3?19Ûn@·Þ?ï÷tBòîÊ?H+ˆ•'`?,²ƒºî?)¡'YC£·?KTkyÝG?C›¸fu?ï±y³†eñ?ŽÏ™Ú
z?L=ý%¬û2?c¯ø´?Ý³WæZå?‹üüoŒ?ï'pûG®?'R2¢H¥š?f2¯ä¹o?fŸü	nÍ?‰â4†þ?€
ºcP?ïèù3>c?Veýfè(?GmÙD4Šú?<ý¢Ïã5?a+VåÓЕ?RUü-Y÷»AGN4FGL J0205.2+3212¿çÍûÃQÆÀ<†Â&€À9#T˜Þ‰À<
qÉp÷º@\b}x¦°@kÛñ,þ?«°
ÏK'?²)­ß‡ö•@S¤!²Ø/@<¥Á›p¿ÊuIRk¿åò•ž¸<r¿èTS¿DÎç¿èQ°''¾¿ì1Û¿ÙÊ6¿ácA&
AGNfsrq3FGL J0204.8+3212B2 0202+31?ïø>Z;
?B¨i–s«¾?'TÚÏ©Ñ?·]±&å?I2‹ôç‡\?@¸$¯0?ïèyPl	?jˆâ¯
§d?3ÂیˆÁ™?Cl©YÓ'?eTeŵ?gAȟ.¤?ï·ªùé:—?tB\õ8 º?ZÈÀAYׯ?_RêôL?}xRøüzÂ?rRà.ز?ï÷É7–ð?3îl=/Â?*ô…¥ŽÞ|?ŸœI'G–?J¶
Ì?1Üz—t¹q?ïñúþ'Q—?P]KuÕ ?1
·[r?$C1,éÕV?Wȁ~dÈÎ?MÐy-³â6?ï¼12b±?ƒ´{åWë?Bã6ÎáE+?T"I0.?‹£k#Â?'»½¿–hð?ïu8y¡µ%?…4'õ…?c‹Ù¸¦£»?f+"¸sÛ?Îë*Èåé?ƒ½oΣHe?ïçWsôh?V·j4Þ `?GˆThI
?9z«'Ö<?bÆvÿL?SS°wõ¹AGN4FGL J0206.0-0958¿êzáV,î‡ÀP[2 f<uÀ;ˆv{‡_ÛÀ<ÊXÓÖ¬@!Tÿ™Ó¦0?üámÙ!næ?Ðrñd0×
?•ñ{ؾr—?Çn,ÙQëZ@%v\'É¿áî=•ŒÄŸ¿ìäÚEÀ¿Û̘ÊfÀÿ¿¸4ûï¯P¿ãŒÛE5"7¿à!4-.6tAGNfsrq2MASS J02061590-0957174?ïÓúéj½8?—$·ÔÉï˜?"Ö¶¸gÕÇ?~'ý Xä?ukՋï)G?—'»;òù?ïÓtVòˆ§?t͖\áu?Dõ½ À®ç?OfbÅ·ÿ?s§Ô©?r1|+÷?ïeïŒP—?~Ž';½q?TzÏS¸­g?:'>R,ØH?'úaƒÉ:Ö?~Kºa¼è¼?ï /#ÈËÐ?i<Ù=:i?0©ÅSˆ?@1ç5ü?‡nèòÆ|>?i4¨à%È{?ï¬é£Ø§?ƒ'W¸›¸é?1Š¥ë0$œ?%­ûÃSù1?"9jžž*?ƒV ÒÉ=?ï•R};?Ì¨#oý±?PŸÇÿ4S?`¥%†ÔÈR?ˆ—Š'?Œ4wÝ°j"?îÇm¶Ö…!?ûäǨ?[÷Ѻʥ?Wg†í߇á?¢°|Õ«¨?ŒÈ[á?îËöiˆ?‹kbå؀m?Cµ(RU†+?:»¸ýòw$?¢ñÄÍÖ¶P?‹tÈá}*AGN4FGL J0206.4-1151?îiàS'NLÀP­[[ÕÀ8üQo^]À<(.Ï÷#¸@mO–U¨@TdÏ?¥
¸À¦N?¦'ÎI#µg?ýUúX R†@P+ÁÏâ¿Ò×Gd˜…ó¿ãlh'î¿åÞûmÊö¿ãPPzkÖé¿é={Uá³å¿ïÿ3òuÓÂAGNfsrq3FGL J0206.4-1150PMN J0206-1150?ïõëòpº?FߒUÕ¨b?)#rgR?<éOäA?Rž$4Þ?E!ÄôO?ïîÿ!ç9?fÆɅt?+Cf—ù0?>NûV#D?^™OÁç?c†¢FÍ?ï²×ÔÎà	?zõ^°GW™?`Ó´"Š&Û?qòŠü9Î5?~*;NüA?s?é)
½?ïúÕKvuþ?(ÌÎ4|s? `›ôzwv?^<B¢ê?@'«Üž?%¸‰e(£?ïëLä#y?S퓒««?7iPdƒ@?)mï‰	Ý?aÅñëØ?RdÀ¶ùWÄ?ïÏ¥"¼¤¥?€‡ bÑ|?>ƒào´"ò?V.#1èðA?vDø&ʞ?}cdšÞ?«rÎÃ?'2º\Äò?h¥îÒè?s×[¨ªÒ?‰jt¬¾ÿ?}Æ¿…ÿo?ïôx×1?Dž41G?4®,S" "?)ôÐî÷Sú?QäoÃiÇ#?@t^–ÜAGN4FGL J0206.8-5744¿ÖOF¥¼ù¬ÀLP64êÀ:ÌÁTɅðÀ<ÅZã{dû@·´Œº?ülA÷ò…?Í7xý—ÅÚ?ÆæÇ	i`A?úÀÇ¯;@ÿ¥' T?ïÿüÚ±'Þ¿êM"M1â¿ÖKž¤pb>¿Û¥i±t'¿àé"89,q¿ê"]u&ÊAGNbcuSUMSS J020640-574948?ïÃbõ\|Ç?<çÏÎ.?A¹ó†zŠŸ?VýÌ|K|??|FÐïP@?ŠÁ¸8ït?ïÔZk—Žä?p,¶nrîš?B4 "Ò‰3?Eqàuæ?sŒ6W/'?l¼^،ûO?î›h†?›fS«žf?bŸª«hç´?pO»#8?¥…ÚÖÞ?›ñŒõœO?ï¦WaÞ
ß?^Ñ×M•?N'=a¨1•?1+£,áL?"®\à†?]­àrûÛè?äá¯?‡i"MäÉ?K£*Câa?Pbs>pf
?ˆ$f¢)?†=hpuÁ ?ïL•ÚÈ?‰&ÞCË9'?P•`¹y?YjÄ´l?‰ì@ȁ•j?‡{ä‡;Ž›?îIZ€Ä? •éEZPy?f[Éý'2?p!¤Ì?­².Íß «? ¦¸Úà2?ïSŠ&ñ?xãso:?[ìh›ó?K˜û'£y
?›]où‹gj?x6®q#ÐAGN4FGL J0207.4-3855¿ïê†;mê>ÀQòº`À: r̦6`À<´zˆ\Zt@5ôå?_@Œ|½ÀÀO?¼J^¼?¾g:vÉ`?ôšøÄ¢[à?üòUû_1i¿äÐG«<#¿ÛnÂÊ £¿åÇ]Œ£¿ëÒ ;I?fßހ(A¿ïÿõ¹U ÄAGNbcu3FGL J0207.9-3846PKS 0205-391?ï82Ï5?–àÄ°:ô?`H_sç±?]'j|ô½ð?–óó(íd;?–!‰°j­?ï»l§?'ØòåX<?Vð.|nSX?`žoÌ&˜Ë?|éÿŒäg?~Xcк@?mã2j?'ùe××42?€¸¬Ñ§Š?'Lü…î?¢W}ðdº;?'+/S‹µ"?立côœ?hÅºDÄ?Q¹|üëz?A…7bŒ?ƒð°c‹‡?gOµZwh??îrèþE5?¡œ¸Gë¸?x6ñ±9?{¯"'«0Á?¥¿‰:£U_? 5†&x¤Q?ïF¯썲?™'Mª3Ãò?g'ψÜ
—?sçeýÒRš?"E$è»Ân?–Ù`v:Ùk?퀴•äÙ?œ_ð/ÇP´?‹n"]D©¨?ˆÚÝ»F?°Œˆí''"?™Z(¾°Âe?îêì¡ Ç?ˆ²fŒTvJ?jÏçdúÀ?dÉüe?Ÿhhk›¦Ü?‡Báڃ¢?AGN4FGL J0207.5-1049¿ºˆˆ@®=ÀPr½f'|À;^ìz>À<—6>@!¯vz° @êE%£þw?ɲN¨Ú¿ƒdZ¦gr?¼ 
|xˆ@ã9ÇÝû¿å™‹¢
+}?îñŸoÇc¿é‰Êï|û¿íJU^×&?ã_Nyà–®¿ïúÛ2ÁlAGNbcuPMN J0207-1047?ï¯͓ØK?'¾BÛ¶Ž?Z¿:^ïØ?zÕkkƒ¾?€ãåB'g?x.÷¸~y<?ïßÿæÄ^ƒ?r¸'Ô" ?=P'Áõ?Ncúhñ?lV
m¼¦?oÍ->­\ë?îٔ8†¯1?ñíx?qMì($è?vbƒlÙ? <þï ï?*Ï#£¥
?ïàêiÑæù?YÇÜþiA(?%™ï]?
æ].9×?n"iA¬¯‹?Y‹Ì³?ï_z@…Mª?û"ã
÷Œ?`\ýû_‡?`Ëñ?#Փ?'4È3µå?‹úL#ÿj'?ï¨ (¥¡Ì?‹ÒÜÏ]Y?Jœ¼ÿ:ƒ?\'ˆ~fÔË?"N)ø,½?‰où5.M?îÜð}ÎY?˜§—ÑEìï?~׏'¿hÁ?'B#6¡â?ª·?{Q?–×
¿òxø?ï"~Û/ï?zÂÏ,c-?*ëêé iÑ?3PFcdÀ?Št™"m7?z›HaøAGN4FGL J0207.5-2402?î®î·Ð‰ÀR$œM©?À:F´ -œñÀ<•S–€	¦@̓P:@FúZ¤'D?·¦53h2?Dd!×Z?ã€e`WÆ@*'Bðë?ìpÐL´
¹¿ÞJp¼€¤U¿âŒ
¿Ü$¿æC$Aþ¨¿Ô³œzª¿ðAGNbcuNVSS J020733-240202?ïó8èŸ?RYu¡ö•?*_n柆ø?!Agé6ã?VCúA)_?PÜÀÞHŸ}?ïðq…£?cè+-?&8KÐ~?7$‡æ|6?\Vȏ¬€?aÿxØn??ï™ÌMØ?~ÞÔÇM?Tî¹ÕUÂ?Uë­ï?†ï#ÖF‹?}'ՐÛÑî?ïô£¿ÒY?6sîÀð?9jߎǷ?—	bH…?TÔê(Vy?5_u÷©Ó)?ïåâт$n?bÐdè¯??HåO ÆØ?5ÐÃçŽD?f4ê¸	?a%‹{ûË?ïϕ"a#1?|$¦(Lh!?:DŽx(?K™@o™æ,?v"9*µÕ?zOæË&^?ïNjC•«ù?ˆ‡
f¡¥?c©ÃV+-Ê?j‹›ºë'É?"½%DË?‡Ig®ä$D?ï㑅'D?TuLX)T?1ÉMóhd0?#ÀUù?j5PÆvYi?SåjØZAGN4FGL J0207.9+2203?ã²*
PÍÀB¹v_Ø­¬À:ýîðäJÀ<‰iêe;@AhÃbì@5ëÄߘ?ÊθŠJœ0?ÊRøJ~ÿ:@
Vz`o?ÿ2]šåÉô?ÔÚ³àl¼Â¿ÔÜõ8ü¡¿Ëe*§µ¿étËNG‹°¿ÌiýIÂ@Ø¿ïÿ€éŸkkAGNbcuNVSS J020801+220241?ï>›sZâò?D²‡]I5?dëYҜ¬?eÈd
E¦?•&SDÙJ?Œ§í\sÐ0?ïlý~¡Š?ˆÆ¾ÌÌ$p?jïq©Éš?nqÝ?Žß3|ê?ƒÀR(¶is?ïz'/'?‡'ÈÒßcè?y\¶E#3?zlGP÷i?–9€Ah\?'GƒÌy§ù?îT@Ðï`?È¥Ö?uvG'°]?`.·A'þ¹?¨$P7?=Ã?iÏ?î†quRm?›k¨éšm<?uÆec^ڎ?p-Ôì¯Tè?¤àü8^ç?™HKÚZ:D?îXá°+"æ?¤¥:â?~‡øEÅ0Ê?†öLÊt]?¦ åøž¶? ºéWijÊ?îf<ó®ìp?"ÈFå‹??…ªÀùÔ?ƒ,ÄH·±_?¤Wmم'?Ãpçûz«?ë/æñwbH? 9¥0YAÃ?†Qâ¥ðø£?z•ž!½ŽÇ?ÁÛFŸNS? 
…=aÍ_AGN4FGL J0207.9+0953?Ê!ÚóMŒrÀHL	¢@1HÀ;U&£øÀ<a"ÌÐþ‹@ƒÌ_"?ü³^f½¤?Ü~9¡ŒW<?ïû¤$èî@›Ç;"T@¢°çiR?ÒËA&»×¿Ó"2ëƍ¿Ø{{vmð¿è  ‰wãf¿é¸âό¿ïüÒÿ@èSAGNbcuGALEXASC J020754.55+095014.0?íi4!??µÆO'áÚÖ?y§{€¾$=?wß'6??³çuÇ6É?µK,ó+?íì܅¸¢Z?­[NzúV¥?™ÂÛúj©g?ìõý–Åß?¤Pɦdž´?£~°3^Þ$?í^ùŒ7J3?¡Òð"=™?™Ðùñõ?'²Ƴ"?­'ê¾oÿÒ?œ˜g«ºø?éWé¼OY¸?¤<Rqµü†?£Ìökh?Œp5ì	E?ÅÚ¥Ñ=þF?¢¥-ùê™?êˆóK?½ýúŠRÝP?"Ízéøy?6üÑDQ?ÃEà4Äp?¼§Yzžy?ê3µÂ¢°?Ã=CdP.
?±Ì_vi0?·ßý©?½R`ñ˜šQ?¹Õ*ÝVæI?ë×.qú¼?¬‰¢d½q?¥I^·© ·?–°¼Æ¦_S?¼"—.ãËÊ?¨{9>m›?âr†À×~µ?¶æýº%a?©¸.ŐBƒ?ž‡§vŠø?×ãì¦(j¥?µê‰åá4¨AGN4FGL J0208.3-6838¿é¯@4x'žÀGyÂôÀ:oî'B³À<£ˆÁÛC@F¶š[`y@uIÞpc??¶ØrGp,¿£=Fÿ».?îó^ÂC|@¼3Æ«öh?ï0hå¿¿æNèÑQ­¿ç|>¿ÙI]¿äÁgÿBÀÅ¿Í
­B˜ÖÑ¿èÿ[_¢'AGNbll3FGL J0208.0-6838PKS 0206-688?ï×Õ¤Œ¼¼?Œ¡ô%‰Û?B¸æ¸ìË\?M"ˆLŸl?q¾驞Â?ŠßæÎäP¸?ïÍ'r6\?uºû
Yß4?BÉ?!×?NJNÛ|nö?w<ž!®Èu?t0ñ·US?$÷Ÿù?‰0smé?TÔ~ªO~S?@¦git‹?ææö¼?€çßµôˆ?ïØO¹==?S:'°×?AiÞ«ãá¾?)ãd[À#?q«5PÙ\3?R³êcš³è?ï£=ɘ?u}á$?X<ðy½?M½5šÏé—?"4-©èc…?€O!rï?ïlöYIX ?'s«%Ý?Q&'˜uæ?`Ðí@÷?'N˧ú(§?æ8ÛH#?îòÎΐ?'ðzHgð!?b.̆'å3?W+¶€¬?Ÿ`L§ëšW?'y×,X?à?ï{>Óáz??u&xn_†ß?_e_Ç(?Pž-^Ô=?Cªì֗!?ts•ÜeÙAGN4FGL J0208.5-0046¿á¦oÎ͋—ÀLæ…3±tÀ:™ôàèÄÀ<Ã¥Üû@œ=n€@§¬Y¾O?ÀD
Ý)¿~ÀŽ–—m?Á™ÁÕ?þ¶E|â¿ãÑx=Sr™¿âDr@bï¿ål"ABÀ¿Ú5…=A)¿ì4"|+ʉ¿ïÿý±q&´AGNbllPKS 0205-010?ïŠ0VEB?µÏ"‰Ó?i>·GjÒÑ?jVq=êM:?™fãË\?µÌ¾imé?ïÃa'óæu?{!Õ&0k?RW¤hìß?Xw˜Ó?yÎ!äw?v·,í•åp?ï"ˆ"ëbm?Û¼­Ü!?tÎ.˜b®?voG¡ÚNÎ?–{aäæ7ò?ŠPFú=T?ïo€EW?n9^.€9U?l¶?Î?P¿òGÕ\‹?ŒòK^
¬…?jé̘@ž?î¡ ¾üÕ~?¢a_¢o/?}Ž>çÝL‰?uD­&´3?¢4,1«+?¡
eäb?ï]|t'—?'Z™ ?`îÎ'À¤?j<Hã=Q?'2—³¹¡?à]ä'Ùj?¨˜Ô¼?"8eæÓwû?w¸b'ˆa›?w™tŸ}øî?¢¿ù'9N?'¸`6Õá?î'Ù"Žö[?‰ÍC"6‰?ƒ1Ž"ÿ,?p,~5‡?£ú–†?†œ+bÕAGN4FGL J0208.6+3523¿ÙÙ©‡µÀ8ÞT´:çÀ:¢zˆ\ZtÀ<|î¡2ë@ ¬í†««??üä17°pv?Ãìmçd'È?·ÛCÝûH`?önõ›øïk@7Áe¤8?ÑÏ3"f×z¿ßSȟ@¢‡¿ÞµÿÆÜ¿Ñ	žD#E¿áÎW±—½!¿Øµ€ëLê"AGNbll3FGL J0208.6+3522MS 0205.7+3509?ïÛ*¼¨M£?dBHõ™?7%
1K?$…<6Ab?pøPº©Èà?c"Ž ³?ï­âw•?z¥G؝Į?Tô‰ËŒƒ ?W6§¢Áïx?èÐâNÊÙ?wW³T²ˆ?ï‡
W5µ³?y5Xøë?\ÊTú¼ ?T >OÏ&À?Š»pä+© ?xdm夺?îÄ ¶nf?u>él7-5?pkώu‡—?LÏsúøÄe?¡¨z§Î×?tâR+¡*?ï½lŽeÈ?rK,IÅ%û?HšË³P|?='àk|.?~6_Bô±ï?qÏh"Ë&?ï4GÔĬ²?Žß÷XùÄ?cæAvŔ¬?h 9¼ÔM?–ú=0R§D?Œ¶¢ÝÈÅ?ï4 a°…U?'KEG?cµê‹æ.ô?Zo­ëhÌÑ?—6|'‡?n¹ÌÄ?ì|¸aIµÅ?'Ì"KY£=?"wuèÇw¡?l]YŽ1?¹‹N:;3_?'˜$‡EoAGN4FGL J0209.3+4449?ß;7™…‰À/À¯¸kÀ:r™A…ŽÀ<|á®ai@ fŽ›ê'?ü€0ŒÅÛ?Äò™åﳂ?»!²,b‰?önøÜP@@[Èµ¿ÈE»K¿ç³l|*¿Òf'åK†¿ß§üaåοà••_x6¿Ñ,Ó}kÃAGNbll3FGL J0209.5+44491RXS J020917.6+444951?ïšPƒ{0?²¡a¥f V?;PS²êã?jÛ¦†skl?ˆ"|§£ûü?²Íñ"?ïØyJ?ux=ýß7â?>ªÓ°/´?M¼Ìxj±ï?qØÖê^¸Z?sÓA—å8x?ïò±ã½T?yåjÒ£¡?T¡öAˆ´?ZŸbH{m?…ïÀïXo?wkó7|?ï†PžþÞB?c\—PV>,?S•o(,õü?2xsƒêÉ/?‹ù*YâøÈ?c#I	w
Ã?ïsý`ÆòÌ?§€_à&?JKq7±Ý?a®IÂÔï?­øa«4¯?¦(Cqíù°?ï'ß"1O¦?Š;ʗ¤ˆ?M؈§®ƒ?YÐLe^«"?‰j¶š?ã™?ˆÚwöªÃm?ïG-ò½³f?‡û
Lа?_Á²p¡Ç?TÄ…T?•1‹–¶5?†].YVà?î³k¨MD4?lB<sJf?de—Y‰Ò?P=YðȚ?£'썈 ?xÎhAGN4FGL J0209.3-5228¿Ó¾ˆƒi"üÀNb$‡wÀ8—ú…l»ëÀ;º•µßJ~@cŽy*
p?üêzAå}ž?¢î½¾h?žFøaûó?øù5
£Çñ@ Àžìå?Þ5ëŸJÞv¿ÐOõ
ÙwÖ¿âi%]‡›¿Ó­vÛ©‰|¿àKm̌¿ÖG EDØ¢AGNbll3FGL J0209.4-5229PMN J0209-5229?ïòÆAÔqî?O·0â*Áò?!®B¡‹u7?Þg^'?X=³ï (Ó?Mžzm_'p?ïîTY"½?fÙØgtì?-?¬´§Ö??üÏݳsR?`(³ƒ÷°?d&¬‡a?ïŸËÆM½ß?€ÜI~‹¹?U¬®â:¤?Z¿õÿÐ?…WxœOÕ¡?€†a‡?ïÀ,ÐîoŠ?_÷Ž™Ä¸Z?Aª^Ë!%1?(Ü°FÞɸ?}´K»*È?^´ýÁjý¨?ï৬úþ?m®&°#6?6Fi_3±?2Í>ë'Úb?l˜*;-¾?l*lTWì3?ïÉPË8g?C
cp]Ð?AUîÌqæ?SKå Ê
´?yQ¥$©?Ýã=Üh?ïp<§r˜?‡Š¼ÄÝcJ?a¡
;?pZ'éCrh?¼ÈšNz€?…?é7B!?ï|lw¢xæ?wËßL6P}?S$nCßc·?CÄE 'â?Ž€TS]Wñ?v§N­žôvAGN4FGL J0209.9+7229¿ïü-\|@%àŠï³À:ZÄq´xÀ;ïËWÇ@[ZÈ£r`@›ß>¿Xp?ÀºAYç|ü?Ñr»´K¢@í¬«ÅH@;OŒZA¿åå¥ `r±¿Ý§4ø/Q&¿à½¥6Ü¿àŠ#opÑ#¿étNáºo¨¿ïÿ¤àõx¾AGNbllS5 0205+722?&ŸH}?¯`Bž%¿?—ÏáBí?—¹…ס»G?•½+EÞCˆ?«@%‹µa?ï¿=â'–·?†k#?H^f–CèG?T75 D´]?}UB;?"örÂÓ^?ìlDŽö?¦•ôlß?§§k^/Ñ£?œ"†*'?°Ê$"Šs«?ŸEb\Vó ?ïq¬"ŒÙ1?qŠ¯ÌVõK?U¬}¡"Xs?>Žë™Þ?o¥œŠ¤Y?pùY,Ìÿ?íGÀI—ßÁ?¸}¹ÉwÉ3?­"Ï­{?±"]ñŒoœ?›ßÙ%°?¥ÏÖ¦ò?ïM©»ý? ûÇIö±1?d‰ÙgÐ?{҈³KQ!?"Çv'°wk?ÂÆÚ1žº?éÈtio–w?­/¤ƒa?µÓHP¡$?¥Pn6£Ý?»égQY?¤¸`Ç$ž?î;RGå5¾?'Öð'²?q¿Q,Ï/?a8_Š,¨Ð?ªñ^ÒsU?'YGBbAGN4FGL J0210.1+2518?ïþZ'-û¢ÀAWÿ›V2À:ã쮤"À<_ˆü"d@ 6Ä÷@hÑ?ýéXÎG ?Èív{†'?ÂèSX?úþ³†ªª@ †ó¤§ë¿ïŸr÷na?ïD1Rˆc¿½"ëYÕ´R¿Ú`χã¿Þ»S'Å@ç¿éþý×0ÓÝAGNbcuGB6 J0210+2517?ïž*/ÔY?Ž€7¤°CÂ?Lrè׋N…?RØöm±f›?†µÆïê¾b?ŒèÒx¦¦?ïÁbþIh÷?y+Æ2Kþ?Lœ3¬ô¢ü?P·"Ê3ª¦?{ºúoKØ?vX³ð¼Ñç?ïeÜï•à¹?†íôy^òœ?jµ÷
r{œ?wy´'·Œ?ÛFe©¢Ý?'"2€6n?ï.ÈSÛ
F?qlN·8?pŽ@™Óô/?R}ú¹
?–ec|¿(?p\5…*?¦‰ìþ?ˆS8:¢?\³ôêQ?]>í=hé?†×?ï
§N?†\©Y?ï3È
›?'#¦þP
V?a]§¤îè#?kKmPÖ~?—[IÏBM ?ç¶J8å"?ï,œ¸Z?D
¿éâ?rµ;²Þ?zhDiëÆØ?šö?'P?‹Ëõórå?î9©OÖ=J?ŠëÿB¢¥?~Å ÑöÉ?lG³RL†?¨¤rZxb?ˆ"7;ÞAGN4FGL J0210.5-1445?æ<CŠÛ7ÀPõ!…Æ~À;0|ý À<®6Ýß@Š
D·)@í¤Ûìû@?ÉøǼ톬?–C<j¿fˆ?Ê:ÜúA@S>"u¿ç`
¹(*¿åõ–àVÂZ¿äÅêà´
^¿ç²PIÄo0¿ÂªÍ‰
UC¿ïü¨AÓ	'AGNbcuPKS 0207-149?ïÕaÌ"ØÈ?h
Ë6øú"?AÂ$!zRœ?8~x'ü—?sÕi\o­?f‡(Ø+D»?ïÛ¡j¸"?r…áKJl??Hœiÿ=?IIpYûo?p:À¼e(?pJDÿã
?ïY9òêî¡?vÿ\¯Fí?b¥e6†ëê?P萎·J%?'"þèôc?uÍÑãĬ^?ïàôÁ!a¾?P*50Co%?#0¶Å'&©?Ë%soÚô?mØ3ÑÓ?Ouy e€?ï•T·"§±?{@HÙ±a_?Uöï:Sñ–?MÙEÖè4Æ?‡ëôX¢›…?z f³ƒq¯?ï|]\Ò?‰Ûu,
ï?O¿¾ñpŽœ?`Ÿ«$z?†¥°ô5?‡µ í:K?î¹l  Å™?ŠŒW8é.?q+"9×´×?i
#ûÄôG?¢CˎŒ´Õ?ˆÙöq"ÿ8?O'tR?p)!ø?9­ûmJŽu?3Ú{€/?‡NüRÑ}?o¢†Á'itAGN4FGL J0210.7-5101?îô8÷m_ÀNã
ⴖÀ7Žî&¹¨-À;"Ë7¡W@ª¢%.b¿@é¾?kOÚ?"yy»n?µÒÿTÿ6@!þÃüC²Ý@7hÿóÀ­¿Ï'X&`¿áûúëÄ	¿ä¶U⊤3¿å桇N¾¿êÕ#³co;¿ïÿÈ¢› ÛAGNFSRQ3FGL J0210.7-5101PKS 0208-512?ï|²Þd#ì?ˆZÜò?jžGiN4Û?eu^Lei?Š+¶‰‹ÑÒ?"ÝVAŒ`?﹕±òDÅ?…ܺŸ†j(?QiÄlÇ ?ežÙXN0G?~Úßv&Á?'×;ä{Jê?ïW¿»R'?''ýø'"?†Ž!¥Èû'?Š±¥5 v­?ƒï"?†ZijK?ïò;S¾)?FM÷&E«??=Å.¤á.·?2jG»?TÓÀ?@È4Hg‰0?ïz¾Í…¯W?‡<Žùþ?li‰(®°?m¼‹%«gÐ?Š5êUp`??'¦ñ0°R=?ï]üÝ-9–?œ6VçŠ?c"ëJ·l?w"¸'6?'Þ1Þ{IB?›ª~Ñé®?hìJ?•0•×–u?Œ2}.=¥ß?'¿á¢‰è?Ž+à…E·‹?')ÄÝ[?ïãö®¿é?_W	K`*?LBá0µW'?C·1S±ˆ?eÙQ™Vµ?Z9œ|JšØAGN4FGL J0211.1-0646?ïŽrünG~ÀO.œË}AÀ:­ß1S_À<œÂ?«º@bWšÆ•P@ˁ½?ÁÛק·?úàe8?ÝÃn_E°@Õÿ¾^Ë¿â<Þ1;¿ç窟ѿÐ?Þ½:3¿áólß&k¥¿â;‡•‹¿ßPå€wߋAGNbll3FGL J0211.2-0649NVSS J021109-064551?ïñû‰½rV?G©¼
_ë?0¸õŸµ¦?lð7?WÚé>¡<-?E1CæÔ÷?ï幦2ô?j²HŽýoë?3ÃÎÁ½»?@ϓ_"½ž?gÍà@òŒn?gԛ¤<?暴Å4/»?qÐ|ª'?Wø\NàºÍ?`ûxñSJó?'ßC7ÞKÏ?nmOâ2?ïÚEgwÅ?N	ÿÒJ?5ö>X—=‡?]´
qµ?q}Ԅ5¶?M@f;–ác?ïã•8‹â¢?Zâ
‡H=?BMÀý´"Ó?4(•îœ?g×WRá ?Xg›k"
o?ï´¢óÏ3ô?ƒ}_šxöd?CÇo?U:wyûðÚ?¦Áã¡7æ?'4̗ž?ïaSŽaF?€ôì7ã|€?_¶>ŒøâX?ZMÕڕGÝ?'Ú*Lg‰=?€(ö³ÃîÚ?ïžÀ±¥Bß?l
âCmô?G'fjßD8?8êö€ô'±?†Ö­4üÂü?kV9mk´AGN4FGL J0211.2+1051¿Ë¬L®ïJÀG¯Š	ÞÀ7³´&ÚÀ;FÀh Ó@ìœf}t@hG,{Ä?—œM9Tñ…?ªÑÆþùè@¾×@Än@çuK[ž?Á]GXÚ¿Ý×Êâfçì¿âÿp"§Êµ¿àúLÍ8,—¿äÀD=Njſä.¢<ÖAGNBLL3FGL J0211.2+1051MG1 J021114+1051?ïê1ØÑN"?XÿŽ‡Ëœ?:8}xV7?. À^'E6?b‡&•Þ?V¯\4~À?ïÔ%_ú«F?v5 1—+?F‹­G
û?_|'<–T?sÚVñ#ÿ?q惾L<«?ï¨P
{ÑT?ƒu8è‡?Y?¹!øå?_¥Þ·À?'¸Uh/á?ƒ@¶A¹?ïÍI™üëÎ?]‹(l­Ù?AIጵæ?*àĂþ°ö?w1öÚ«ÊV?\CŒëÈ?ïьØ*_?g¤e1«qO?;ÀÁäë{ò?2LK#2a?u}‡Øˆ‡?f™iG?ïžVnîí€?ˆœ¡'N?SNp…*?dË[8Úð?†–Aº#l?‡B&—Φ1?拏AÜ»¥?ƒýbI&áª?\Ù¼¨÷n?kDªÉ~£ô?'ý÷üI;Ü?ƒKL(%?'/xF?uvۗ«ƒØ?P±Lò)±2?AZ½623?‡:µÉÖZ?t®"m3NRAGN4FGL J0212.2-2559?î‡cÑቝÀQú¢‡~äâÀ:þŒjÜí¬À<·†«€L@´Û%«
Z?ý#·ÊÝ"?ÉÈ#š¹Õ#?½.ëÐÉÃ?òðñõ{AÀ@¤ýÒ(V`¿Á‡
`V,¿êHº–i?­¦ŠÃ½Úl¿ã¤ÁëÈ:—¿ÞáAäP÷ê¿ÖޏØO·ÎAGNbcuPMN J0212-2558?ïé'nâiu?TÓÀ†îFD?(ƒH«ÆKŸ?õìàdÿB?eP\\Iôj?Tó¦?ïÖ·ñÉõ?ttË½?Cá—ò?K2'(x›?rCF‡i~?qÐ&]á¬^?ï|¼[1÷@?v&#O_?\›Ÿ›JЇ?^3Ŷ¢MÑ?=u<©9Ü?sŽ?è0'&?ï•wE(J™?cñn¾‹ØÇ?DŸ
©Þo?,äm÷¹<?‰`ô´ß?cÄbh}‰m?ïÊS9©?poy{Aœ?;™›+âAÒ?-{4,Âß?yB¼Ò©'§?oå&GØÕÆ?ï—q\þL?ˆ4 ‡Î¯À?S8§<u¡J?a2N¸F?‡¼"Í/{Ì?…èÛÔ°#§?ï$z;c?'uiÂÉ	?aZU€7b?W#ûK¨?™Ew'-¥°?W~1®?îïu@žÖš?'p͘Ñ{?Q5J2˜¡?DsËÔ/¡? ~ÿ ?'BëJÞðAGN4FGL J0212.2-0219?âGÛ`ZÖÀMDÁ~ºñÀ:åG5H·)À<£zm"h@:iàCw#@ƒýP"WC?Á·ýO0À¿š6°¸'xÛ?ÕÚSÑä@…ѳ'gq?ïçu$oK¿â#Ê|"¿ãÍug‹*¿åPâÁ*Ø¿Ü•ƒŸÝ*"¿×¶ %#ûÞAGNbcuRX J0212.3-0222?ïã´oUDÍ?Y°ãüV3?:*l«"^?%D2
‰?iNø…h,?X­Ð,-¨€?ïßiŽ}Ëw?pPhü'lã?9J~H£T?C,d$³¡?mm!´
T1?m‹°%á?w(?sãôxŽºI?X—T¡ž?BH'ŒÌ"C?‡Â*'?sMÀÜ`_?ïÔ7Ή¡?R\Áúô@ò?9~Aë…:? f@U×<
?tL4²tfñ?R,Ü:>M?ïÇÏaýv
?q˜\Šöå¹?IT[Ÿþ_?8É'¼³¦?xíÛ­fq?q¶7ÏÅ?ï¨>Ȓ«i?…Y%ûg??L$
>ïŒe?[QåÌ]FC?".þw1?ƒŒ¤5ÐV¥?ï4/?"‰J'__D?d0ÛńL?VJgPój?–ùU}ŸŽ?ƒa»!w˞?ï|ÇÂ)ŽL?q½*À5vB?Qƒã']¾?A-ç$áÆj?Ž"Ÿc-?q'`,"{AGN4FGL J0212.4-3502¿ê4xm­‹ÀQ¾¹¡vÝ­À:Wõ ¨ìôÀ<«©f–7@j¶JU @3T¦J'?¹ÒœÅsE?ƒA©ÝMg?ÉÖ§.ë{@ƒC¹=N?ÑEœš*
¿æ·½ ‡_¿Ù`ÈWG¿ÞAàËy¿å³2'#ƒ"¿Ê	 :2*õAGNbll3FGL J0212.8-3504RBS 0292?ï؛·xt'?sƘo8§?@Íô×ö»?-(dòAúb?q˜'Þ»8…?s«—kÁ˜?ïÛÝ\?$?rÊ;Ømè?=åN?}jK?F³ÈAõ?p3ä¡¥Ž?q7Þ?ï'÷ú€—É?r™ð"
ÖÞ?[u™¦W{?UïŠà@äv?‡ÓNF4Þ?p¸(·Ä{ê?ï½c	±üß?X0ºÎkµ?H9é"+?-'*~;–Å?~G=üñÊá?WQ-Byn?ï£Òûî?AfØP_?S•ìM2D?Cq°r¢wÅ?"˜ƒw¡Õ±?~`S0iE?ï£")³ú?‡¶Ú9uV>?QpˆšÃ??`ŸÉ%!É?…	dª9ÿõ?…kÊҗT)?ï5—¹Å‰?€¢-®»G?eà3¸
õ?aéÔµC'-?–'IÅì•?}Á}iöŒ?ïR(hÛ-?uøÀ2$?]p¿Ck÷_?ISë
ö?"ãç5"í?u6HqtëœAGN4FGL J0212.8-2721?—ež·³—ÀQû†ìë¯À:Ìb¯!ÁÀ<·îŠŒ¶\@2œ"uÃQ@CTc.£?Áö
HX^f?¨Dͺ]‰s?ä鋧i@#f•á(N?ïµÖ±R¿×s×}ªÐ¤¿ãZŸ2ਿé·?Ò}涿Ì=$ä
d¿ïÿÿÊPËAGNbcu3FGL J0213.1-2720PMN J0212-2719?﹂º~Û?vÜMÆÎÛA?HÂ}…®šì?A[Œ/?Ɨ?€Wû³wä?usÉ ýÊ?ïÕ87Tf?sxº1¼Ö?Cw)ª
?K4Á©Þ'?rõË~?q5¬U¥ P?ïB=¼R?'šÞ_"°Ä?jzrô©‰¡?m»²
zÝ,?"hú Š<™?ì
µ@X?ïÒÓ''ç?TØéqü¥?Bœ,Å ËÅ?0x#@¡
?tBæú"?SåX+ÑÇ?ïZ"ò§
1?Š« ü·½?^R,Oðªa?UaТ•ÑÄ?'È>Þè!J?‰˜ø¬Fþ?€­?Št˜!W::?Q.ïø8ÿ?\,Ê9Ò» ?ˆõŸÝ^?ˆV7‡À?î‡×"ÍEª?ÎÑþ¦Û?~(ñm"?yÞ\âÆ?£¾è³ˆ-6?ŒÊM@¥Œ—?ïÅ
ú?rXZùº…f?XmÅêÖ.=?O9Õ=þv?Œ€çqç¹?qW¿Š'+AGN4FGL J0212.9+2244¿Öˆžl´&ÀB/ü~k?êÀ9ÐK¨ñÀ<<µ…ˆj@ð2¸9?ÿäçUO?µó8ò9î¹?¾·]¤ËÑÐ@
/»¯n@õÆžh5¿îÑҀ@M?ïæ#J‡ã¿àËÂFa
¿à¥0 Y;Û¿ä<zo1ç¿ä÷ƒŸ‡DWAGNbll3FGL J0213.0+2245MG3 J021252+2246?ïùŸ¹CX?6Œé\*?'~BïnŸ? 6e/Õâ?C¡"§À/í?1z÷ã·"K?ïԈkQI?të)TpCW?E
Dú~?PƯË`ñD?s!ØW›y?r"Çl›ø¯?ï¹±o¬¿?líLrjÛ?U]»³§K?^Ü°;'?yK¸y|mb?fÇ+†?Aƒ?ïŽ)«lwD?e+ð¾U{?i8L[{q?Iù7…Cž€?†''"ô?b´ÝÖ¬ö?ïô;Ðq?DÁP»O1D??"ìßyf5?7Þ·ŽJöá?OIÙ'MÁ?;ùúf^-?ïmM}X½©?ÝYž5s?ZØïÛp¯»?iÁm‡½°?¨Á[¨½ç?a8tÓ¡?ï f=‡Ü?têkÙkæ^?aE/)!X3?gUlÔΨ·?ƒ•$Õ })?pè·û‹§k?îï][ƒg?€hF•,£Õ?|œeD1%?e¯eû0ß-?ší;6Ÿ¿È?|(ßÍþv£AGN4FGL J0213.8-6949¿ç"±/Y×.ÀFÔ×ðí=†À;!ö'õ;À<Àµ™ª`'@"5Wâ¿þ2?øáv<?A?ɂý5uWÆ?¶.Ý8)è?î'gbÂ*@ÞÇÌÿ¿ï³ «Ü'=?ïõf4€¿áÁçâÒɿ؀Q~Í»_?€>—•]tпârá锄AGNbcu2MASS J02135882-6951360?ﳋÝF_?¢j©ÛÊÛJ?8(´q}Ø?S(NZ"?'[ÇîÂô?¡ÓÿhwÚú?ïÚ@f*4?s¢'Í°?:|#' §"?N	Ýkäy?q8
˜•N»?qÓǽÄFA?îÚ¿Jœö	?•ƒK¢¶?P§`ˆ'?TÏýý_Å?¡Ó*ïHËì?•ÀkW¡X?ï­´™­Ä'?i¥K€ëN?7uic¸˜?'ÖΆ§«ˆ?ƒ×.Aˆ=Ø?hí×%·_?b²|¿?`Qý¸Lï?G½9'Þ|?GRË7
†2?‹ÖÃ7iý?óp±‹+V?ïŸò‡$)´?†•ØGÆc?E°Ö_š˜?Vh܃À;´?†¨PƵê/?…]9­OøÉ?î,lØ+·?›ßšÆžD?R4cQÇ?PÕ7+ô¦4?¬®&(á??›ÙÌ?©?ïõ\)?†ôm-]ŽÚ?Km¦€#¢?CÔeñ—¥?žڅS-Ó?†ø÷Ϻ$ðAGN4FGL J0214.1-4733?ïÇrøÅùõÀOù
¿cíÀ;€£n.²À<ê»ð¶ù@ qâ;žè?ü#æt=¿~?ÝΟ C×Æ?·_Kêå?Þ±]û³À@ßyw»#¿ä¾¡@W%¿ËâäfF…ö¿ã[ºÜ	€²¿ÍÍâK ¿ÛV,\\׿ïó±"L["AGNbcu2MASS J02140989-4732357?ï0¯ Ê˜ô?¸÷Փ¯p?XqÆOZà9?|[ÀW_î–?˜bï'gŠ?·x«Cp³?ïäkÍzê?l>…¡h
¼?6/`GN?Cóoœš¨×?i¨< ë?hë
_rP?ïm3)xu?'	Å¢sIY?]-þNÒ±u?[Ô±ÊæK?†ºó9H?ÃtςH?ïËÈ]L?Yõ?ùÂ0?/ÃK›Dr?ªEÝ8ke?yu|qú?Y©|Z­lS?ïЖŒã—ƒ?ˆ¡ö·Wh?6ŒF,$è?JuÔÔ•Í?vT@¶ïT?‡&TÅ­ˆ_?ï¥%ç<²?ˆ?Ôj
?J¶Mi†ê?\
!1žP?…Q`á]?†RŸ+¡:ð?ïÊó-ߌ?ŠµÕû¤Å?bÂòõ}µ€?`®{¹kê\?.C2¥[Ô?‰Ñ]fs¸›?IZù?w%tÕ$?<?2üžâª
?0üvEÑØ?EHÂ84ª?w6‹Mj²ÌAGN4FGL J0214.2-7025¿ÜÝ&bP"RÀF[ÕìlÀ:)?—Å"À<vׇ:òD@Å´Júz@Ñí@	ÛK?¹g'Ñ_Ú?°¤žìzù?ðB'!¬øò@?q¯ðž¿Ü€'q^çí¿ç@D"­Ç¿è'&ëý¼¿èéé¾4ú¿íA8D,¿œµÐ±Þ´×AGNbcuPMN J0214-7027?ïØJî!Œ?gɾϯèR?OjF`Õڕ?AD Ì+k?oڀzÊݛ?eM]K¢¥8?ïUÍ!äà?œ0;¾qr?pw!üRl?uÏtƒãA?']ȗÒf?™¿ZRĹ?îÌHS¼ü±?'PoÑkh?ˆøcÿXæ ?‡Š—.k‰?™úÍÛ`¾?ŠY¥ùÁ{?ïœN+ÿY´?fÖUÄN]?r{â'ìR?X{ínPh??]Tùz¬?`<xj7E?ïœ]"'H?~µW-@†?a'"†\í?Uú×½Ä¹?""4CÒü?{õEÃ	?îW±0°ç?¨Ð¶ã…?"^
-c[1?"äˆTÑT?¥md¤ÃE?¢I C='º?î-ÁúêJ?˜%Œãp?ú³r°7?Š²ÈÕu?¥%3xìø?"K®o¸¡Q?î¹z¥ìñ?6œ|Örñ?uÐP_ÊÞ?€Yi•ÕEÀ?˜ZÚòw?ƒIY¥4ÅÁAGN4FGL J0214.3+5145¿é0ó;ˆÀ"s2&ÄÀ9÷kÅJøLÀ<C:8
2‰@ ›ú©ÿÃD@ñ›¹.Š?®CµâO•ê¿´'HnXÎ"@7E«I@ÑZÚôã?ïã)›üå¿æ™Sù|X¿ã«xßdÔì¿Ô±qÝ=r¿âkí>\\!¿ÏÑß[DÊAGNbll3FGL J0214.4+5143TXS 0210+515?í´ŽÝw·?¦
{Ýë?g*fïlñ°?X«<7ølž?±¢5༷º?¥®ÎRrŽ?éѺ?ßòw?¿–Ÿîa5ê?y0¹
?ƒ?€¬wEõkF?Çï'6¸gª?¾x¬hmœ?íðHÿðˆ
?™ª+Ã.?pb\âË9?d)`q
ð?®ï$b `½?˜Ë%C5¨¼?îCL—œ?ˆÔ&J|?ˆòîMÌ?f=9†[fÀ?©¶Îw‹–?ˆˆzÜkۃ?ê$·&Ùo?¸ýzWÏ?F5ɝ?o
½F:­–?Æu_yH|'?¸˜ä'¨?ã¶{'ϸ÷?ʈjÃÔfÛ?†/Ì6ÔòC?"<}iCá?×á‹OÚ?Éß]dlú?ëcc&Àß?©GTˆ?ƒ
2ÒõÈ?y)Ú<̍?ÂaÏFt¨?¨-ßKœº?éª(KèO¤?¤Q
ÔWK:?£½Gw!š?ŠMåXbV\?ďï\à?¥xZäæAGN4FGL J0214.4-5822?à眄¹hÀKÇߏG0@À;}ÂO›HÆÀ<òÿ4(%¹@\E*¯}?þû˜\'·Ö?ÓG÷›,–·?Ԙ\bq?ýëWfï"b@
ôù
†¿ïQ¶
éh?ïÞ'bEo¿Ü—û3èe¿âÎcûR¿æU.enâ¿ïÿü¥¬¨AGNbcu3FGL J0214.7-5823PMN J0214-5822?ïöG¾kÇ5?G%c‰h"?17.ÔT™?+ʊð- )?NEo'88ß?B(2u´gD?ïá3}Ÿ¬È?mk5ÓØvý?9$®ó­'?F'CÞ=
?k§ìv•óo?i0ˆ;«Û?ïIìiŽþ¥?‹|îÊäþ?sõIÕÎ^‹?xú	'9Pì?'Å `;·¹?‡¢ô°B\Ú?ïÙv¶Pñ?QÇtz{ž?G­î0RO?,¨&¨
?pƒøZ?Pcœè¨×?ïëZtž@%?c ñLhûJ?EË÷o¹?Cé=0À¢?^ñAE¬?^t—®"G?ïš0"»'?ŠK_Ó8òq?S«­Õ%4è?kj©çy‡?†þžÒÈÍ?‡:›Ï÷s?ï
ô»ºg?¡`ÂD?yÝ]ø³wh?L(MU6&?—Êÿ5?ŠŽ	ü¥z?惡_~?læ'aP,?Rï¾%¬m?C
8
¦V?ƒÿâ3w^?k݃ùQ>§AGN4FGL J0214.6-4333?×xÕñ°ÿ3ÀP Ž4À;ïiÃèø|À<ü]¿Î·‰@"Ù¾9a«?÷ Â'Æï=?ÚrÁ`'?²Ì)cы£?×"ªú¿ú+?üøÃñ11?ï¨HSUèj?ØãŸAyG¿êcnÏÁsÓ¿ÉÕ	‡=K¿Ðu¬¿ç<¿Ç""7ª¼,AGNbcu1RXS J021439.0-433319?ï|,™;$ï?…€†K~Ç?8BâÁÁVþ?0™¬°r¹ç?aE­BË?"Þ3¶í²?ï·eka?ƒñú'Õ¢®?X{Ù_Ì~?dñIc3F¢?~WŒ_Ȉ2?çUyX?îÿ¦Àëåc?ŽÑµÊÇè?`ü3(Àu?eg¶â›'O?ë¡~^bˆ?ŽI²õŒéÆ?ïs_%Ýé?…ºéoMs?P§½ãi¶?E^)JOi?›ç?¡\…?…‹•™ªL?îó:Í[h?šrÏ-事?FkhEŒñ?<èÍC|ú­? r¥‰ÈÞY?šRðËjÞ?ïgÓxãk ?–æ»eé‹?_WÔJ"]?pcÊ%bÆ
?'™Eþë?"×Êkno?îjÙb\k'?–"µØ_?:?bA䡶»Â?i儤ÍþÉ?¨.K'Õ©5?•ý#=%/?íûìcÚµ?¥ÌRu
¡?]ú¹š?^4µm q?¶Ü'˜u7?¥í
AÙ"AGN4FGL J0214.8-6150¿áj`û‡94ÀJN(ܘëÀ;6¬7+xÀ<ÄR)˜¾@Pþ39é@ˆwîN&Õ?Ð|³úîÉ!?Ð>͛(åÒ?öýã¼Ó[?î—õøó¤Û?ìŸÝJÉQî¿Ìôœ_ÄW¿å`¿'țæ¿ç[`m~¿ïÿ Êƒ+?ïôìp×±AGNbcuPKS 0212-620?ïs†E»?®x
}£6?z‡ó.l?…~•¦Á?—'v
/?ªØ~…Û?îBfÕÞ?±¸aà±?—P®8ûÇ?¥MYAh?? 1G6$ž(?¢áúƒÚ¹¡?íÍwäàa?¡8·²'up?—9p'xãÎ?ö)Âe?ª†p:-V?›ûõ5Js?ì­WÿåÓ?–¦_"ï?£ÈXmÜ$Ï?‡›ÁhÊכ?°±Ñ̙?Ì–N¿r?îð:»ä?¢*q
v?‹½£7{A?Œ°Lþ$L? ""0žå?ž£›ý¬Pœ?ë$CÖwÝ?ÃÝxÛLÜ?°Iƒá¸?ºö6÷@œ?¶"ÌË@_?´3o~	h?ìµ\a¹?¤J3'rèS?žÜóØ̬¹?"¸ªÿ6p?²âl…à
? ¹pǺՄ?渌wƒU?®·(³$?¶Å>¥6˜´?¤@V}ØKp?ɽB|bO?ªç3Ò×AGN4FGL J0214.9-3722¿ï@lüq¥ÀQip£×
=À:Ç	á*QãÀ<¡ jْ®@»ˆçÕ@S3¹jð9?ÇàáÂ'W]?±>lwL"?äq|^ö/@¹U¹ÅÞò¿°ˆUà˜lÚ¿èæÙóü¼¿èyÞp¹&¿ïÿ·äkO?ïîÑk%¿ïáûÓJ•PAGNbcuPMN J0214-3729?ï~Íîé_Þ?½JjËÈ7?kœ©ïª)?™!½~ ü?‰l#k-å?·oÈæ"f\?ïË/?''ï6QFT?QÑÚ¸#Ç?dï5©Ao?v!}«ŠÞo?~‹v¼¯ÿ#?îÛI‹tE?'}'œ¹Î?nBKfG=?r>-ØÃ_˜? gAtíÒQ?>\DK?ïøѹ#U??®­Ùãõú>ó¬Ì¦®n>õº¤Q»â?OCUúæ]??'•£þÁ?ïï"ÔI)%?k7Òþ??Ô10&Ì?Kµõ˜d?XîâÊDÅ?e]¼ ./?ï|pÙ±â'?˜ƒ	ùí±
?`îFÀ"äe?•ÉŽÕt?Œ¨7ÚpÈ?•ðQèÿ?í×ËΛD?˜­£?|P،Rò?yªT}Ë?®ù(
•õ?—*‹7äÅR?ïà{n©?eØï"=¾¼?G,'5o?"
JªaA?nǧÉÞ?eƒùÇq6+AGN4FGL J0215.3+7555¿çå=ð..o@+ÈÂ?«ºÀ;)A® 9À<˜?gôÛà@"cÑeõ?û!DˆÆ¿?ËlØÆU9m?ÀDc²,
?õ#|ÜÊpÒ@'ÇœŒ=;¿ïÿîͨ"ß¿ïüúAzÓ?ïÿÿ^ðP`?y7»ûe³Û¿å&Õ!/$±¿k7¯çUAGNbcuWN B0210.3+7540?ﳊ"v¢§?/àÒ¨?7úUÑ¿F¬?*1Aü²Y?']ˆ*‹5Õ?áHi?ïò8ÛØr?¤Æÿ6	/?g'Fãå¨F?nÞ¢=|?E?™üÐâ¬?¤$Óýv@'?îMzKÅ?Ýÿ'§‰¨?_Ss¥€5ý?b£ié¶ ?ª-Ã!qL›?Æ
Y'%?îWF˖kè?‡Ñ7¨~\ÿ?e+Ùé"¸?V/B`ÁA™?©8Õ§škÚ?‡³fÖ@?ïŽÜ,ÍN¹?…ÄK¥Ä?C#û=MLý?8VÀ_†?‹µ*¤›?…i(Þނ?îÃ9XÄÆ?´mÒýGÐ?r©'Z±"?€XgRÓB?­nšEÁv?´@(!!Ý?í›(Æ%q\?õŵ
'?c]önÉnÄ?aDÓ¤‹õ?²‹Ê³æ?oà5'5?ë]Ǭ…L?¦0¦Že,+?y‹ÀáT?xO7ýp¤E?Á¼ƒMÌ4?¦8ÎcûñAGN4FGL J0215.9+0300¿ïäeh±ÀJÏO'õfÀ:Ÿµ<OÀ<wRœ…e@›	³Ýè~?üðÏÆ|P³?ÍJ‹¼[?ÄØOø:ä­?ø¨Øœ
è @)_SL®.?ïþdŸfã¿èK7 }£ð¿Þߤ¬ó¿Ò¤^Ƃ;¿ævîÿ|¢h¿ç,Sæ1!áAGNbcu3FGL J0216.0+0300PMN J0215+0300?ïÛÐU?fœ¶1
iÏ?1àٔ·È?&.²G—Ô?qX
gë×>?eÖæpRɊ?ïÄ4`Àñ3?uGW6+Þ?L§ë¼l¸?RFŸôÁü?zPÒ(þå?r¹\q¶Ì¾?ïW󼥸6?…sF0¬iW?]ý´œºkb?atŒ°Ü8?"!­N–?…
Ú¤ŸÞ·?ï7CPë2œ?nJ 9Ð>?_䍹1©Œ?C\$Hñ?—M	ò<á?lø5Å*ŠL?ï½lcÅ;?p^5ð*_?Ar¬r!?7ó6kç?K†Vêû?oh‡!|i?ïf¼½Í«?‹ˆd±é?W¿(lBÁ?aX¾ƒA:?'¬{šmi?ˆÏ©×òs9?îÝt¯vÈ?'hd˜[,?iKÖ?k
¼ú£Eÿ? "ø͊ ¦?'ùcÑ3?íö@ÒMë?‹
³¨²'ï?nÛ/Maèì?]I±ËNÓ?®®K+HÃ?Š9jX.,sAGN4FGL J0216.5+2313¿ìXügçgÀAÍ®_ú;›À:'{&ÁÀ<deÀN9I@ º¦'Ço?û)—Ãք?ōK±?Ç@÷Ií@Z	`ÑÑï@=*WíR¿·²Ãa>3¿ê‡/3Ê1è¿Øì]Ù¤÷¿ÒHj|öu¾¿à¹Ã_eÁ¿âsè/(âwAGNbllRBS 0298?ïÁ¸ì	ï?hY[+Åæ?PÌ_UÂ?</ðºÀ?{VÙ0Øm?fÂs¬î2?ïyü§J?ŠGŒ²F?bî–V\?bÙ¹.@[?¼5	~?‡ÿJíFç[?ïo›ÜiøÂ?u¸ZQá?eº›«Bgœ?euç ׯ3?Žªaíú§£?qÙĀš¾Œ?í¶òRöЊ?ƒvû=ZIê?sªãPl^?Xß¿§Ý?±
¿2|ÌQ?ƒ,ZžªÐ?š"ÍØ?zæÛ±4•?d‡—ñNƒ?Uy>
a|o?Š¸óvæ®y?xpgÅÎ?î">1O>"?¡$‰§?uÜ 

<¾?~`U´t2?¥˜é0à¼?ž"¹ÃyŸ¦?îŃx? *_'—n?u^±gFÛ9?veŒ½æD‹?¡1žÄ?Œ†¨_¶ó?é˺éþê_?ŸdQm²•?†j®©Œ?t€P¿¹~?Çhý­ÈÙ+?žê©¼xvAGN4FGL J0216.6-1015?à1ˆŽ.sÀO䦰)(À9¯'OH<°À<Sû!sî@´¹¯ä‰­@ÑÿÁìžú?²"¡9öñ¹?¶"^—&@rá& %9@/«$ÜX[?ïØ~>õ3¿á[CÝOÒ¿â(ey×\s¿à峃O«9¿æN'b™R¿êdüAGNbcu3FGL J0216.6-1019PMN J0216-1017?ïõ"ª°S?SÀÁÖ'm? vddþ?é#õ!bU?Rç݊bV¦?RGgÛ?ïðYNe?d#ZôÕkã?'ØÛ¿»Ÿ>?:)•òF™?\RHÕbnÉ?b–xÜnƒ?ïÃÒv@4_?ió¼¶æAÏ?QíÀKK??™‰ÈÉ.Á?y›T¸F¶{?iǃPô?ïï܃ƒ?=a\°+Y?1ÛƉºÀ/?ø±\w#_?[ÐñþY?;3M­VŒ?ïñ¹wÇ?Rc«çs?-—ú,)•z?&Þó"qy?Z)]BE¶?PpîêØË9?ïÑ+åï?~!,ÒO¶?:êE}‹²Ñ?LyêÛ_?u»ÌȐÀ?|ªéá¥2ê?ïšu¨:?x$÷+Ö'«?bgƒÓÑÒ/?cô×ÍżÖ?"߁¾E?užRYGÓ¬?ï×h-®Ñ?Zu¥TÖ?F6ËrLE?4zÁ®^?q…ؒä+?XŒÏ@£håAGN4FGL J0216.8-6635?УCf‡ÀH2â\
WÀ9ßæÆsxÀ<A,…šT@ˆ€UÐÁú?üšÊ¡yaì?µ³›ÎR2þ?ˆÇ#ël @1'o°'@Oìú"±'?ìÕsd{ª›?Ä;å'Ûg¿Ýá\†Ô¿Üi.âìsÜ¿âžaÔU¿çž|øy#AGNbll3FGL J0217.0-6635RBS 0300?ïóæÀ~?G<G	<wÃ?BÃeÑ.F?=?rÆßLð?M¤CÙyFÌ?;³j‹xô,?ïÄ|i»Ž?zÕ»%2ÿ?P¿Ké?[R^ifNÕ?y'6ëÒ?w^òÙÐ?ï™Ï!:ã+?'¾«;Ít‰?tyw$û".?{öµ¹íÅh?~žøR0G?u킫g¶–?ï]Qµn%?l&ªö°@?jвkìÇó?M¥`ôö?'_}`uX?iA~â ~ÿ?ïã®óóØ)?_\ˆ>F?\*"éC?TۗàmÓÂ?\wö_ÛñM?NzÑZ®—?ïQª…WËÌ?•¦³‹ò·Ï?bÁW·@°_?n¹£ä…­?"r"XŸm?"Þ0à83?ïT‰–[Š?üWtž?…¥@K1*?Š™û4¾?…8Z!zR?1'£It?~~'‰?…ëÄãg?zYFS‡¢²?dèo¹úú?£oP¨‹?"5æÙuÍAGN4FGL J0216.8+0510¿²×¼o"}úÀIÕg–ØõÀ:¶ÿݛQ*À<"YÙU@ñiî†0@­õcÄËw?ÂN´XŒ´?W.0ͤÏ]?•ü‹^öä@…>œÈÎ?ïóg ù	l¿æ¦I«D¼È¿èZ9œÙ¿ú¿¸
¤ô–•X¿Ýв_Ž0¿ïþÖ4T›cAGNbcu3FGL J0216.4+0507NVSS J021655+051018?ïÖ-|B¤H?hP"Bý+?AÀž"†/?2"م™Ç?r±.ŽT%?fòšæBŽ?ïÖ²+êG?p‹…=·0?@°×©?Ä?EƄèiVÍ?rÞض
?m²v-…~—?ïjèS†T?|ö
‰½›?`²áú;†ó?U܆²s?Œ™\Ü´?{
h
kÃç?福«[™?aŸÄn	ñ?N¸D(?3AGÉH•?ƒøÉ»W|ç?`í¨D™@e?ïÂ@·h?w¾wÓà?Lßl´
Ÿ?EÆMøØ?{D÷Ü1z?vs'`o?ïÓ"¡åÃ?Œl»ó"??Nã5ØÝ>€?_1הÚ¿?œëp—eä?ŠJ‡
I?îîÄÆîçT?ŠÛ1!\²c?iy( ªê?aŠ}ñÂ*€?žøB$o ?‰–]}sC%?ïX$Ú*?€'˜ÇÍå?fABAMe)?U_11…ó?›LÓ!w?~ù'KózAGN4FGL J0217.0-0821¿Ñ‹v,úVjÀO2q`•l
À: ZUÖÀ<t¿û-2h@¨0lYoˆ@+œ›¬™Q?¼ð¢…?À•ÙE¬¯@Lz-È?þ66ò?ïÜ3<mn˜¿ãb€u¿å0éý_;пåv•ˆ'á¿çŽc_öµ©¿ïð"¡!1AGNfsrq3FGL J0217.1-0833PKS 0214-085?.ú-?ªà@É?am҃×y?rp"˜{ý?¤~O>m8?…•'ÄÒ?îäíÏô	?§9Vۅ?†°Œ?âð°?Œ*ݧ¥ã?˜	ÿÞ*ƒ?£eEø.eÉ?îË:¢#'?'©É]C·l?‡í¥ÞÓ?ˆ½Ð¸?š¡Ù8}æY?‰ýØ¡ý?í÷[8,c®?"ÛρÚv‰?—פyîï½?wÜn`qä?¤žz?ffI?}Ýù±¬h?î-zîCü?·ž¼ë+¨=?|ÍËÖ$á?vˆ±'$F?©¥Wc¥R?·–¦ÂÂg?í_HÈEÔv?¶6¿ú×L-?šýrZ[-]?£p2Z)Èú?¬ŒºKálü?±Š78ìÔ¬?íNX'ß\?£'x6 æ? ¥G©‹ð?›÷OØ/x?ªu7@‡OW?•X)ò½v?ê¾ÚæëÜÝ?Ÿ×ˆôxñ?®2¯á¡É~?"¤pÃÜ?ºïÐÕ<Z?–	ÃÿóAGN4FGL J0217.2+0837?â>^ˆfÊÀHQëcÉÀ8­43ä3À;é=~æì@¾»Ú(Ö@ì·M߆ä?¤	±ãÃ?¥]™@áÐ?ÿ¶¢Ù´;Ü@ÈBS6³Æ¿Ò¼ççÛF¿ãeøí½]¿ã»'Ê°h¿âë¹VÎBï¿å҉øÌ¿éJñáeAGNbll3FGL J0217.2+0837ZS 0214+083?ïï׍^ç†?S»öµÜIÝ?*"™&â ?å"ÉE
?]'õ¿–û?RPŠ‰ÖQ?ïÜË×ü£!?q=0›Öñ ?A7ˆ–¤!™?O@+[åsé?næE½!$½?mkM$Ѿ ?ï¯Ñ×x¢S?zÉ/ðÆĦ?Z{6Œkú?e"ՁX?€¼#Pù×ò?x;héÿß³?ïÚÌù(±‹?R]¸Kò+?O3¨.{?4ìƚt?mf÷×òV?NlÀqA…4?ïÑusÓ?n
ùݺý`?A¾º*•v?7ç荼ô?u
ƒ`œÛ?kòEpÏ*?wѕ+?Ž•Æà«z?QãHx¢{?doînÂßC?ˆÉjØì?‹wj¯F56?ïw€r´±?†t:E"`"?a2ï•su?fŽ<	˜Ê…?Ó'|=4¶?…Í%¡Ê÷}?ï­os»?pbM¦öª9?b'"^Ô®?S"ÙâB('?ÿk­½…å?j̋1›àAGN4FGL J0217.4+7352¿ïÙ֚àì@(âCV–æÀ9͌æ,ðÀ;¨Ó5œ™ÿ@—Èe^ÿ@tŸM¡?²ÒRȤÉù?ºÒ	!¼¾7@Ý¥b$¸@
»ž8¥8¿uv×çvà÷¿æïÖòÀ|\¿ëhª¾¯þ‹¿ëÕjËOõ¿ïûâ~å¹-¿íÏîõì€ÇAGNfsrq3FGL J0217.5+7349S5 0212+73?ïåµù™?rY_á¹Ü?bQh³Ð?qÈ>`úy?Pai·TéÕ?Hr(nÌ1?ï#¬ûK:f?¡—cpw?€AV«ÃÒ?'Ët}Ã_?"iµ8Lâ?˜ÍbnÁ?îî'é!P?''&?'b?†@,ï5þ ?‰~¶g¦D‡?—
¬ii å?¥ñZ‡a?ï&
zÏ¡`?xó¼'ˆÇ?…""
­2G?l´†°äÞï?|ŸEžæ?ov_?ïÓî÷¯?u4WÄô?mLJTÐM?soÑùwDÄ?]‹ÁM=y¡?]í¨•Xõ?íÈ ¥Tä?´×ŒÂ#Y)?'ð3ØÈú?¢Gáeí?ª}å­öE?¯ìõÍ|>"?î>àï™"?˜=·kr±ý?'¹	:U*?Ž5îcbŸ?£ˆ}E*K?"¡¡Ÿ˜#?íU>\å'?Y/vY0o?£»Ô¿Ðß?"åÃÿù¾Ö?¦òWVñ+æ?dkQ—(NAGN4FGL J0217.8+0144?×=k†òßÀK5 @|ÇÒÀ8DôètÉÀ;¬šˆ¬âL@ÍVnjñë@FÙ='©?X,€«Oé?°X(àôÌñ@Èí_‹Î@ƒxOÇéc¿½ñ¾xÌ¿áU74I³¨¿ã¤ô xÆe¿âŽWF7ò¶¿æ~c³-¿V¿ìì¿0|uAGNfsrq3FGL J0217.8+0143PKS 0215+015?ïðm'dt?L¨\Þ©˜?7KϊÓWÃ?-I–÷öåÔ?Z 0§ˆ´¶?H¿—:¼—½?ïæþþʐ?gÈžÈæ?3œ¹Ñîþ?>ôíö8¼?f¾¡;Pš?e£\‰t²?ï¹wòø'?|¨{œöö¸?^C›ïbˆ?k£vþÁ;÷?{³ÅË,?xÂ56É?ïõ»¬Ðd?8"Â
v™[?!T‡ –Å.?
ÊHOùƒ5?R^: ú?6ñRˋ-?ïÓÔ\§å|?kMAt½Ý?@AÄ-dAœ?=¹Ë·î®?t
™«ÿ¶?i,PÕ(e£?ïÃc¾&§ñ?ÚI	и'?Hsôt½C?fØÚhÁ?{?¢lýàe? "µ1V6?³àí–?…uÄM-w‹?]Ýڇé¢?jŸÔGA?…WÃ%þ?ƒËóKj?ïëc7ª2»?Qëe"nS?1 úN{?$ýµÔp"?bhÅӔ«3?PÁYÕs	nAGN4FGL J0218.9-2305?ÝàÏ"ÌûÀQt_®¼@ŽÀ:"WÀ±5˜À<žù˜òc@"ÆóÄÞA@˜Ã`<€º?Àb–P9?¦À#Ç‹Ö?å'"^#̹@š?Ĝý¿ÕfÓP0š¿è,ÀÞ'¿è2µ>»§‹¿àÀ;Ÿ=r|¿ïÿþªJl?äcãÏßAGNbcuPMN J0218-2307?ïû†O 4å?4×Ñnԝ?%àõU|¶d?·§¦{$®?8Ý‡GÐ?0𭿃?ïï[0c†H?eZŠlUjÍ?)pb™ý?9Ô%~I¦?^"Ký$ž?c,ï¼.?ïƀv¡¶¸?jè녯_ß?YW°È©?c:S¶|þ?viب¤±?b¼Ê*ši?ïúÐCț?)•ª_î:?Ø1ƒÇU?u‹)w¢Š?Aä¨Cý?'pc¾W=ž?ïø.Ÿr?C¾w»kÓ:?2Ÿ'ñ'ó?(Å)8Š?q?FA3vÖ?@úbõ£<?ïÄx¿Ñ´
?†PH»-Z?Do5D~?VVÙ#œ?{5¾}ԗ?ËJ‰ð'ý?ïžÌ76ß ?xñ3ŸÄË?^^ýÔ/"?^¦Dº|¤?"g H?vôÓÙàÌ?ïðƒxÅä?LX°ß"ó?2³¬–±¤?%wô9?[˜©4?I©>¸3 AGN4FGL J0218.9+3643¿ì7ƒžtc™À6ê1…ýÀ9œze ì	À;˜	ÿ÷@¥³/³ø@ʅ4-?¹¶ˆèœa?ǤC@Çpl@
f|¼A%@``?°Å¿Àß]ނÐ¿änôËG<¿å=ù*"é9¿çÑ`°D
¿í>"z~K¿ðAGNbcu3FGL J0218.9+3642MG3 J021846+3641?ïώüÌ"?~×"š|?e	5ê
àÛ?mqɑD
´?kgÎ;#üæ?pž©:®Í?ïÝé¯?n¬/6î6?>ÿXwk,ö?Da\}%m?o
®;H ?køõ)@K?îø*Ïó"?'Ñ2ãÞà?€ˆñB-e)?€±ï$J<?˜¶-dlZ)? ‹Z€?ïAá™/ø?t›¯ôþÞ?]5ÀªuL?Câ³WÜ©?•ðpÉt[O?sSJb¡KD?ï¶GµKPá?vèҁ¢š?oÚQ4{?fÝ·šzY?tï­¬m&?mÚ±ÿylÝ?ïÀ¬ÐP?Œ0÷J£?`7à !—¯?ué^ôÇ-¢?‡êWĄ̂A?ˆ6»£»¤?î
¦"WÝ{?JÞVª40?'W€¤¾z?Â"2Ù8n?¥ù݇GA?—ÊEUl•?í¨Ð•üxƒ?"Û²ìòt6?y¥֘Á@?eò©S–˜?±+Aáǒ?'ð…=àîêAGN4FGL J0219.0+2443¿êœ°ÞÀÑRÀ@ÿÊ}g3ìÀ:T6KìhÀ<]°<sMÕ@ {ÂqÔ¯?þBÙÏÏ?¹jàHª"½?œ}¿ZÑæ?åT*Ã@LÌQ#ß¿ïW‡Üóö?ïÿ˜0ã͚¿äQ™_â隿àcRµ¯z¿ÜJ±ŸIÜÿÁÈpMLAGNbll3FGL J0219.0+244087GB 021610.9+243205?ïàºDßØî?[G©G«ò?;âáÏyãŽ?='öŸt?kÉ^ÙÙ=‡?YFL;ì´?ïÌÒˆê?u-¦é"ÂÇ?BBrÒ%Oú?Hüfµ0‡K?wN¯SR×û?s}zVt?ïu"f—?yÃ0]j:C?^†:C¬'ë?Uhš£MÛ?ŽÊU[ù'V?xóMºÁZ?ïc® 3^?léÏ¥Ž×3?a­©ïn·•?C™ÑM" G?'Tv¹j¦Y?l1҈•Á?ï´C¸€Sf?u.}™?VaòN?Q­Ü€Î¹b?€+_ì-?s>…OId.?ï_	̀žB?'¢'fñ'?Q¢Â6—©?YË-»§ú?"
ü©F>?'5[×l8
?îü*O??‡žJ'Zy?j$
{¶?d÷vˆ	[Ä?:V9³Û?†n4EiÝ
?îe¦¡àÕ?‰Ãs¢¹ÿ?uï!¦7öˆ?b~D%Œ=#?¦çºžà?‰fO3Q¸›AGN4FGL J0219.1-1724¿ïft€Û\³ÀPã9–ú'èÀ:Œ/•ïÀîÀ<€šl'p‡@74:DI†@ÖßZn
 ?ÀZâ9E›ì¿m;8€Éç?±cDë@ëÔZŠ»¿åPVY¨é¿æ%»`"¾Ž¿ç)%]‡š"¿Øë/þË¿Ôx=({¿ïÿÜßi‡ƒAGNbll2FGL J0219.1-17251RXS J021905.8-172503?ïÊ$Ǔ/¦?táª%Â*1?G³ÃGqB?F'=jœ¾?w÷#é6`t?sC¥#îû)?ïâ¸Dæ ?vthP?3N®ÈmÆ?@¹D%£¬?jÝåpT[?uÉ`E_Ñ?ïwâk´Gà?€ÊÐC‡èº?WÙepùæ?a.™P?8Z÷^?€1ƺ¤­$?ïÌàtäc?XúÜ	j´Â?0›MOFjÅ?Û#[á?x†Ç͂?X¬Yݽp?ï{¥Õçþ?+Wá!õ?XœèÏ{ï‹?QKp)å?Ží|7š?‹´"êPf?ï±BKe?[?…wnqXÏþ?Ep#€ˆuþ?XIÀ-L'?'XjßKÇU?"&¨Ùþ¨?îÁÓù"&'?•V=îÍþ?`òpC‹¥M?`ÿùxf?¢Ó™mð`Š?"|ØcR•?ïj7ùí`?x:cb¬Æ¾?H]'úúl?<Áó.#<?'ö6Yž?wêR^9£½AGN4FGL J0219.5+0724?è«Óœ¹xÀH³é ÀièÀ:ôBŒüÀ<cÀ›f"@ YC=A@mY9?È/Á#K^£?'ûôW«7§?ÎõŒI$M@¶ÜuŒI?ï©iñ5aâ¿åÒ%fÁÕù¿è¼Çf[~¬¿Û¸‰ÿr¼`¿ä ~æ¿Ûš©CÛ¡ýAGNbllGB6 J0219+0727?ï˼¸ÇK?"Œö?"FÄ?:#‹BZ	?K'S˜âœ8?xjû•ÇÜ?'âfCì?ïÃ×';$¼?u'	LS?JrÇpǘã?Q'UÍnâ§?zÆ{WA?rõVæ
i?ï†DÉ]­?|pÀâÔ»?V@R¹¼t?A¡a‹&iG?‹·ì¬@YD?|é<Fèª?ï©ßÖæ?`ۇ¯E*<?Eÿ-ÑV?Ä?)øÆí´J?"[ÕAÿ?`ÀdÇpeš?ïšä«ÌÞ&?1zä´2j?DCpZ.Ö?6m4pPô/?ˆüñ%ô?~V倜ˆ?ï|³`ÙÎW?‰‰Vü7ò?Q5yƒ¬vÜ?Z;f³hM?Ž¬x£½¥a?ˆ¾_7"J?ïEàp(î?‡@"ô1?að•Jõ²¢?[4±û<?šÙ1O§^Þ?†##aŊ?îï"Ÿ^¡î?~´ð´öÓÅ?`b€ÁÇH?NfšÐ×
? ®K,ä?~"$\FæAGN4FGL J0220.2+3246?æ¸i OÐÀ:z|¨"2À:‰m–cÀ<QjúIݚ@òÞÜĽ@^ڀêv?Îj'ÅêÛV?Ô:è‰A@s¹»x³@øE×î¿¿à¶l¾o;ø¿ãt°¨©Ø¿ëMª½Ù>ö¿éx՟eæ¿ïÿå(
eC¿ïÿþÐñAGNfsrqCRATES J022048+324116?ï̍
Ù¼Ž?r=
"Ãô?^ûGý¤??Ur2'¿""?r7;ȱsÑ?mµ¸"¦xf?d'¶2?ƒ"·™t.Ë?fÖÄ%Ã?jÙ+/Ñ¥_?†qWÉ$(?æ§þ…?îÝûȇ»?•
©gÁ%?'vaõ€,±?'7P:¶Mo?›mh"[J?'$½±‹'?ït<ÎpŸ?i¥«Ê˜oñ?r§Tñˆ"Ä?SÀµgUz?‰!àæºS?dµ4P¦Íë?逸^&"'?€îèÎÀ?gÿŸ€?c|W2!«m?€ ·Ö%¨?{Ò
Ô[Ü?îÍɘð?£©¸¯5A"?4µ'ò?øUD]°"?¡Õö	d¶A?ž‡Drð?îXËÓÓ|>?˜Сۖñ?‡IÎ(*?†‹Þ¹ìòÈ?¤ Ï<"?"¯¤Sú¡?©§6?†ì'·ë2?†à®gB?§?q[Í'³?¡†z‰Ý.²?'uZ…AGN4FGL J0220.8-0841?ïà&˜°LÀNúˆ&ªŽ´À;SôÁœ¬À<´ÚìJ@–@!–L\yþ?÷Π/µÐ?Ôê&yçL«?Óú†c±Ö&?ÿ'~þà¹@W#	ðCÊ¿äúTû½¿ïÿ"Þï?ïá³äžzª?ÒÈÌøk·¿Þ~½_ÇeÛ¿ç:d_¦ßAGNbllRX J0220.8-0842?ïÊ¿ž]p?}sMÉoFË?='"T[?Æ?6ÊÐÂ.N×?xÈq°r×?|å8qÀ?ïÛLkÏ?{¿øÖþmp?C´^F}W?T^mli³–?o춥*µÎ?w}¶aûî?î7Ûš*?ž‰]ÐM‡?g¦ßƒ*èÇ?p )P?«Õ߶'Š?žèÓ?aþ?ïP€s5Š?|Y&¦8?Ay)¼jz<?4¦¤Ó¥š¤?•q¦žUd7?{ì€Ç:¼"?ù2'è?‰|0Ô¾p¯?M>g0Œd?G–¤p>?‡}[<Às?ˆê½b?ž?聾*Ä?‰çæ'ÅI?Tk
hi
?jNNj?".}'ë?†©ªJü.?í6ìÊ)j™?¤ÆùÄ¿?gð
"[?o­³UM&‰?µ‰Bìð¡?£ÍŒ
µP?î{o'fD?•ÆÓ "n8?J}`þ"«©?M$	Ð[s(?§å"…<ò"?•È|C
AGN4FGL J0221.1+3556¿ÔôÙ/º5À7|K	éÎÀ70–›¸XÀ;)ûbó@Žn F±ë@Çâ'@¸?ŽÁsR]?¨¿3\"ë'@(}@@ Qg`Œ\Å¿Ì/
3Å)j¿àå!×¿ågûý<a¿âý§*{ԍ¿èKABG£¿ãE5þAGNFSRQ3FGL J0221.1+3556B2 0218+357?ïè²­"È?WÄ®¾ïgu??uÉ¥¨B†?5ßȖbk?c^™Þte?U2éyeM‹?ïáêë"-ç?n)YÄX;?:gA2׳?J\«»{ßÔ?jÈ,pH¬à?l­€Ò³v§?ïr‹â5?Žwçږ™?öÉqà?†	…îI§Ç?ƒÏ‹ú7Ô¯?†M	Ú0?ïú°µ¿êç?0Jǀ¡XJ?
µµí4x(>ÿèÇRàš×?CaÎN<Ô3?/
ߌŸœ?ïÑCñé´1?s%øƬþ?:EKH)?5"xOu?u¹²Wš_?rÃúR+oê?ï¾eyèŠ?"J95ˆÿj?PåwæXöz?lel~ õO?|"å'rì?ƒ'žîÚÌ?ïb@ñ{œ?' ŠE0O?€wÆè{?ˆO¢Pÿ?†ø·…i–/?‰dªŒv"‰?ïó¹U€T?LÕ8P³\?!‹Ïw'"^?&üj™_å?V\S¾!ø?K›ó:Ú4AGN4FGL J0221.2-1312¿¨%¦ù@­¡ÀP4 {5À:ý‰»Ö"À<›óÜ܉@ÿB%¿WC@òa|ÚQ?Æ SG$צ?°¬°L¹l?ä܅§tM°@l6k!=?ã¬X]ºn¿æš·¦ÊÛ¿çuK;gµ¿êUü¡PÈ¿Èò]dŠ¿ïø^졬AGNbcuTXS 0218-132?ïËé0.¾?©oÅ1÷¢?9•FÉó"?)üúl?xr!lΕ¾?©q§)}'v?ïÁ÷Ņ?µÁÕ7Sx?T™D¥š…‡?aèõVi¨??yÝÌ-ފ?xÚzÿâc6?ïJ]g ^k?€Ä
9ÿt?iÐجË@Ù?h,ÁQµÿ}?"z7ü%}?~Ä?Uòx?ïЦ"¢¥?W€uE¦L5??U?È Ú?/`<É÷?u·bd´ý?VVÞ~¾'?ﴘô.Ä?z{ÂÞ×OS?Js¨ÈNvz?AJ8B3"?2Ľ"¤‰?y×ÛȌüö?ïqЊF•f?"fNœ"ém?amíØ1n?u)e'ø‰?0•ý‹d*?'_BüA"?ò&où?ŒÌ(á@d?wv†·ò!©?uºBw?¡§	Dn¼?‰b¶nì'?ï`i½'y?y"¹êý!o?ZÜ]Ø[ó?Qo:Æ¡ü?'ExJ=?wÑFþoóµAGN4FGL J0221.5+2513¿ï0^¶³t¦À@¨û¼¾bÀ;>1ø .À<Ò2º¥@œ9í±?ûåɾ$"]?Е™"Ë×.?Ú3~݀¤*@
Ô'ܾ²@	G¹¢£ƒ}¿ïÿÿ" 5•?ð?ňP†€7H¿Ù¦¿<@x¿ä"éõҀ¿ïÿô!O…úAGNfsrq3FGL J0221.2+25182MASS J02212698+2514338?ïÇö¹&Ê?…TÞ¾6¾?SW•ÛL?Twó­êe
?wžŒ6×?ƒÚ˜|TÝ?ﳎbXåŸ?'[c<4?T£b¦Ùj4?bqJjéJ?€‡û#±¼Ï?~*ôëÞ—?ëVž-Ž??¯ñ,¶jj?£OF½"CË?ž/Wp$6]?½e§±º!?¬bÓ
³Ë?ï[iAÚbY?p<&íÃï?k#àõð§Þ?PI÷ùšP^?'.[¦ýâ?mЂ‡Vè?ïR1¿Úe?""‹('ü?emõŽÓf?dܤÕ8¶h?†Ïö,TD?"Á¯E6?îù¤(¾»?£rÚI)m ?sW¬›ö1?‹·ü7ë±?œ
¤þåiJ?œÖÉkgƒÒ?ëªÖ—?»ñ?«›þïKâ3? Y1ªêF?˜Þá/+ýå?º|Ê/RlÎ?¨DòàH.â?qây?‰ÊëµÀù?w{æ­¬ø?ivñàÂÌé?¤T /#ÈÌ?‡"ݳK‡ÃAGN4FGL J0221.8+3730¿ç<çFB&
À5÷Yš¦	À:àÐd1À<m?!Î@iohی@êS%A)?ÒÇþÜ¿^$?Ø*Œ»º«¸?úÔLJémí@Édm<ïJ¿îLAœ''?êÿý¥\Æ¿åº<;ðq¿ãU]Œþ¿ïøª*s?qInAGNbcuGB6 J0222+3731?ïkÜ4HÜé?Ñsßýh?fü¢>5@?a±áLÑ·?IÊX¼O?ŽÁ{åór%?ïl'–VT\?Žz³YÇ=?rmç!?{¿á'/îR?‹ÚÏ@…ÜA?…	D/+}?îÅAtR&?'Ãm‰‹X?ˆr¶•y?'£,'!}]?›WSñ;8ˆ?‹°0üû}_?ïÀÈKw'?{sÊ¥ô§?{_e‡ÍÄ?_"d"Yb?–0
ª[µh?wwT`Ð0?îý;nYéš?"éÓaÊ?tî®úI÷·?p/Òho7?›æ}"wÃ?'EÂ=ê¬?î;• §Ú?®}žq‡¼(?Š¦C·j?žpˆ#`?¥)?¥:^yÆ?íõVœÍ?›óÓÄ/;Ï?ÃB /¿?‰
+^†?¨Ly—zîN?—6 <OUm?íEbô}&-?˜'/ÊÕT?'äoZö?}'—.cJg?±"cáC)à?–gövxßAGN4FGL J0222.0-1616¿ÉYçû¯ìËÀP—æî·`À:'õˆ­¹À<8Uêî @éÐ[L¬×@GڎVo?¶é9"÷ƒ¿sâX'Ö'?×Vj…YñŽ@
mc-ת?íëw²¿¿åY àŠÄÀ¿çWeÂ|'Ì¿â€3aV\-¿åû]8À:î¿É_A"ÛAGNfsrq3FGL J0222.1-1616PKS 0219-164?ïêͪÜüµ?ŒÃ/4ãñÞ?'|õe
?‡ÿÐ`¹?cº…ål1Ö?ŒÀBö=0?ïè÷‹oèÏ?g§y,ñã?1!uEʃJ?=)®TlF?däF)œ¾ã?dó–/?ÕK?ï»Ô«N³þ?kø«$ií^?R$â,@ô?:蕀ªŠ{?}ŒqÀ °?k<c8?ïÛ¡âq~?J™4áûÍÐ?7!Õü.|=?sóÌÉö?p¼ñd"á?Iò[XÚê½?ïìTgx4?`é¾~b'?76¥ñŒËk?%Rx|eµ
?`Å$Û)M?`¥@™¬?﻽§&0R?ƒ,Î\?ED0)À",?X*‰mˆãÏ?x¦JÓ?'voÐtÛ?ï"þžoÛõ?~h¦Z8Û?Z!PjÐ%@?Jº©s†G?‹|.NÇä0?|ÌÚ["1û?ïŒ&êÙò?pMÊiÂO¿?Tù,Zà¤?A!äXÿó?Šu¦4›S?o™0ÿ®vÍAGN4FGL J0222.6+4302¿Õ¨Ò?05À0Ãúñ€À6¢7Q¥åÀ:°"±"L[@Y³Ã¼Wà?þPKŽz??¸ì^ý*?¦d'‹‹@Og+ˆD@B{Ÿ]©¿ºÆ}A8m¿ØPÜfrÑ¿àtÐ!#~¿ÜÈh¤".M¿â4áô|>?¿ßuAË|jµAGNBLL3FGL J0222.6+43013C 66A?ïÓ4y¥?l~ålå‰B?9¦žh¢'?2Ô±¡L)?tËYlÇ@S?kë÷§BVî?ïàŒâüäí?väÖg­õ?<acËÜo?P¶´[x?kápÞ
‹µ?u)5 ü0?í¹ÞÌ9?¦>Î??vw¡ÿÿ?'ÃÝ·F‰?°Ëþü·Û€?¤ð¥Í·?ïÝ°`k¶Ä?[V	ÎG8?&Hë	å@?jó"	?puˆƒ¡Ô‰?Zë¼­ïÌ?ïx2Þ‰3?ƒM¦ÈG5?J˜²#3Lè?Cþ0Ú!?$Þ¬A­?'Ï'ªÂ?吏­)Ä?""–»•XG?S'>¿ê?lšà¡ù¢?ƒÇÕoõ7¥?"RŸ
چ?íɸ¤æm¢?¤\ê"Ì5¬?q0JÕw$?€‡Tñ¡…?°Ÿ6-yåé?£¾¬ÁD?ïõH:› ?rR\⺺ó?2{4LG×?,JŠ•n¤Ú?|ý¨¨þUú?rp|F!úAGN4FGL J0223.0-3447?×ÿÝá:ÀQ>þqŠ†×À:ù]Ø"keÀ<²Ÿô&­ê@`À"…b@4:<;ðq?Ñ+ºûéñ?Å¥o±"‹?ñÿPÈooú@	û2:å¯?ïË^£#†¿Ó0¿P‡Î¿çšß¿Ø¿çkº=©î¿ïøô=Te¿ï;f›ÖAGNfsrqPKS 0220-349?ïzuý]8j?'ŸúÂå~†?e"ÿÐ¥Šl?yV/²VF6?Œ@¨ÙÖà?ý'ùè:œ?È_Í?Ši'_52?lHAQtâä?uR4òMTe?†¦ñMð?'¾ˆ"ÆF¥?ïKxƲ¤?ŠÎ«4¦Ä³?}¿g×{6¸?|ŽÙ?Ø?–¶é»¹ã?"eÔ¼š›?ï5V?»
?r‡~˜›?€Þ¨¶ÿÆH?d1_Ž§î\?åèޘ¨?lf']Yè?ïN[þ·H?Šk‰á¡¸O?iJÎhÙâM?c)ƒ˜æ•E?"&cfã¬?ˆ7-'nWD?îÒ®½\S?¡`Žè¿_?|do<Þ?†sê9m¢?ž'…´`?œÚ¥±nÌ?î!†b…0?"TpÏÞÀŽ?…EQöX^?û˜©W¿?¡Ü"5ɲÞ?î¸Æ4Ì?îƒérä"?öû¼§Ð9?ž"ÒÓÈ?}Á·¾]?¦(wÜD3î?‰+Ç%TÄAGN4FGL J0223.0+6821?èm
îïÑ#@ïÏ_ND1À9ë¼&Œ[ÃÀ<Ê<ϔ'@ —W´?þÉÎeS@ð?¾¨*+!ÁÇ?¹Fho*/S?ûàÇ¯;@E®CÊ°¿á€À_+3µ?¬–ÄŸÊ®¿ã.Ò{bw¿Ô.iàCw#¿âúã±à¿á6YSXmAGNbll3FGL J0223.3+6820NVSS J022304+682154?îöðaÒWü?ÔJ)Ý6?c?£,'\?T{¥)ô§?ž¹ÿY€¾›?Œ™ Zº÷è?난[9?¹ú{HÛ?u1zã—[?z‹'Çb1?ÁLÂÁ?¸.E3	?î™P.û?‡¥÷'j¢À?sþÔì1ë*?`§½zÌ[?£ë#~N(q?…·[ïkk?íðm9Ù?X\ß;PÄ?‹¼t«ßá?f€o"Ä?ªÜ'¿©Ò?}šã¦ ?íRi"ï?¢x> ¼³?{Lò£î?q5"øªR"?³¶µ'ÐU ?¡K_ÆViƒ?äºê8åÇ?ÅÛɗ¶@?‡`ýó¼?"b3[4º?ÕÏ*–gÇ ?Å)ËQ2Þ¶?ëþåFÒ]—?¢Ãþb•"F?†æZs†7ý?tŒöÑã¡ø?½,
}H?¡´K€ïÅ?êÕL«²Ô\?˜™÷eç5e?¡‡öˆ?ƒ¥'°K(Ê?ÀgëŽP\±?˜\zãTÛAGN4FGL J0223.1-1117?Ú ¤).f_ÀO¡Ò|96'À:6–•[À<}Hé}Ý{@ f&áÁ&?û*|«LI…?Ëkûf=K»?ª×Äøm?üàÝ%	¤Ä@\PÈðIT?îI=@}H«¿Þ•ØCùT¿åµmÕÆp'¿ ûsÿ+CÑ¿ás~§Ð¿¿æb»K›	AGNbll3FGL J0222.9-11171RXS J022314.6-111741?ïí+ú@	?QæEY|y?'@)—ÿ<Ã?k7oўÂ?a…ÑC´Ÿ¬?P3"7ÿÛS?ïâMõ×2+?kn¯²ø÷¶?6Þìd¸V?A¤Èøë?jÖ,°ÙÅb?h¡j¹&e¼?ï¢ì¸
Ú
?rÖ@8á:F?Q§íµ­?Tûês[)?…ÞR,Þà?rØjœwa?dyv?fIXÜ‰?NEÜå!ª¡?8W"Vx!?‰uI2lòn?eª©AÝd?ï×ÑÊÚѕ?e‡K˜ï¢}?9Ìø‡"P€?-Ž³RféU?rzK
Ãe	?dÁ{䓚'?ﭕҏ¯`?ƒ÷e»:e?I°8j	¹w?Zlke#C?'ÿ‡ÑBlÕ?'wQ¤o+ù?ïR;ì?'ÙÃÍï"?ZWML´#?^ª»"‰2?"|o¶H?¾•uGRÃ?îå•É*€Ý?÷ã4þé?`Çü
™$?S‡õ;ÛN? š#«v}ð?ÚúÝ]·AGN4FGL J0223.2-1653¿î \ë#¶$ÀPœ!ÿ.HéÀ:¡'&цÀ<,:ñm–@aĪêNé@(Fya?ÑéQò;?Ûbs'žÔ@	¬s@i|›@	("ÌUX¢?ëÚ7ïZ–O¿Ù1¥^ɹó¿ê"÷€Õ}u¿í+LŸjéÙ¿ïý—ÛSxM¿Ãˆ´oõ˜AGNfsrqPKS 0221-171?ïÏ%Ý_A.?{ÂD84>?nߍ}Ü@µ?v
Ÿ¯l?aú"ðYt?gñÐwcÓ?îò±ÌÕ?¦Ðt [˜?ÂŲ³8?žfx±¡á?"#e!ý1Ã?•¿7f]R?íÛ¤Âd?š"›‹rU?›GÃG™ÅÚ?'Ðgˑ‹?¤«ôĪh?"Œõ°ì}‰?ìÌÆç§æÜ?•×ãßÁz?™>§äÂ-?{	&ãÐ9¶?³JÈà1˜?"óbkb­'?ïŸ{f0i2?Šà €lç?€| ²Že?†WWJ¾?n'ÊE(Á?sI…±
žœ?컔ƒZ=
?¿@f¦Áå?§FEÏ š?µ0N6оÍ?­Ÿ‡ü*Œ?°ËöfÛ?ìåâ‰â3?¥K|·'ø?¢ŒK¦'="?™+}9ða?¯‹Ê§m=?èÑ.>(p?䈘ÇÙë;?²;òœÛ'?¶"äW•Ú?¡$¹3B?ÑfHwÇ4?²ü߉ì+AGN4FGL J0223.5+5415¿ÛD`™À'oÀêÁ5¿ÕÀ;UZ'ÇÆÀ< ×Ê,ß@!níËuì?ú½ý¬h©7?Øy*"é9?âD Á@§@=\œ¹Ë@}µ…]w¿ïä…CÛ¿ïÿêњ'ç?ð?Æ´ž˜1Á¿â¼œW~¿æ¤À>IëAGNbcuGB6 J0223+5413?äE'Ä›Ùm?×;?JBn?Žð4ÚO†?œê0#ÍÿA?Ö}XÖZë?ÖM6û|8?èIyS±‹†?í6¥bê?uݤù¬Ø?‡RìzV,?Î+-ˆ×Þ?Ã9RWÌÖÄ?ê:ÌÀɚ?°ÙõæÊÅy?~Ëà!–
?{ù›îÁ"?ĚÎm5ãg?°Ûq?P?î‡O3ç/œ?ŠXÛ^A?cȄøÿƒú?T
¬ãÌ<?¦N"nûe…?Š¥}îçV?êdˆsè–=?Çj÷¬¢"?x
t Ã?‡&qýÊûÏ?Å­r&r?ÆÜVýµ÷?àؾ\"÷?Êîíˆ7?š"¼q?'Rï'óV?ÝÐÍ¿C«?ʄÄÂY×?çœ÷âÐ]?³â_ ­?"ÅOsϓ?'§Lð©Œà?Ðç×?A‰?³Ý'tq?ëï8Kç×?©¹(Ä?vª¿Þ\)<?u2^óeÖ?¿"_ëð?©€2=ÜAGN4FGL J0223.5+3912¿íVÔc«1XÀ4BÁ HàDÀ:†câ'§åÀ<yˆ¥U@²Š}òÊ@¾4[Q_n?ÃGÃx4–?¼b	4‡=?ö®…ÙÚ@¶œ€SÍ]¿ÕÜrÝGÅ¿á‡gÓMðN¿år5a¶©J¿àyêaÞv¿ÞD]·ì¿ïíE]'<0AGNbcuB3 0220+390?ïÔjÇ7ü?l€
B¡­?CˆrR?aSÈTo$o?s‹<FÂJ?e
cz¬¤"?ï¼û'6b?xrçv?Pª…Œ-`?TkB™Ü£B?}WõíO÷¬?v«ì[?ï†pBÄ[ö?}/ú§8?\\­Fžñ¯?U=çmí+X?ŠØYµãX(?|[ê¢ÐÃà?ïG´ªA1¤?p°b' J?f,é±Î³q?FÍèý%ßç?"C̓WÃ?p+!Ì1`?®`Ðû?›u~µ§<&?g߁!¬Ý?™ósaQo?"ßô&?ö3?ÀÊüa;¹?ï5ÿ8ãT?•Cr¤œ?e!>Æ飽?sAp‰'&ê?–›ñ	Xs~?"¾ÀnNû?ïXFƗ?…=í=³ÿF?mëùu½Àl?n¿Ûæ°Ïœ?™uË*?'Î_¨=í"?íÑN³†¢?ŽÉ¯XjÊ?!BÆ%J1?hL%>ö,d?¯ìl›?®5vôAGN4FGL J0223.5-0928¿ån>LjWÀNÿ‰?¯BxÀ:ã‹+AÍ*À<¥­ç.wã@$£ÞlŽ@×:ÿ°Nè?Ì
,"óŸõ?Í4M¦‹ð@ð÷"0{É@(Ätñ¿ïÿÞ!ˆæÄ?ïÿíáoq'¿ããªÿójÆ¿áTî~ù/V¿é¼êº:#¿ïö…Î
ºnAGNbcuPMN J0223-0925?ï­ÿF
•?{ÇÝNx'?gïaPjº(?b"J"­?}¬k=C¸?v¹ñ'!Õ¼?ï´r¸Ú&¨?'_³âÈp?`i¾'H|?nÊCÞ楝?}'Ä'¸@ù?zŒbqŠÂ?îé¥)çýL?"AdŠ&?|«å–†5'?€Ñãöu?› a]2Î?"ôŽ5L
?ïò]—œ?r®~\ï³?~T©Œk1Ì?^â•jA³›?"Œ"6Ñ?o÷ƒñšï&?ïP•,*3
?…»˜ÉšP>?€1XÉ5	Â?v:Ù7ÆÃ,?‹©\+æ<ÿ?&í4`Æ?ïÝ# ÝÊ?'ìÔR?x·otU]?™ÅiMO?—v³öYg?•7ÕF}n¿?î*ªý³ä7?™g8Iq?‹nj5œÓ?‰QÚ6Üz?¦yÌ	XnV?•$ãý$ŠL?î~]×?À$tˆÐå?ÒAyô˜?x…? z"‰?¨ƒŽ,ƒŠ?ˆØ:ò¢ÒÜAGN4FGL J0224.0-7941¿ëtrúÀBAþûôÅÀ:liÁd¹¾À<|Jù"–-@J&>Ù@%Û[ÛÉ?¹Û©´nÝ¿™1¿ìÞ?àæzÕéV@Læ/ŸTï?í"Þ9Û¿ä©Q†¿å
$¡u;¿å¤=ÔÌË¿Óþ_o×(¿çˈ>¨\UAGNbll3FGL J0224.1-7941PMN J0223-7940?ï´ð?B¶?sU³{Æ£?L½{COj?;²µÂÔ;î?€ølhÍ	?rL×ôDQ?ï´Äé?}l‹Ô/?N	èè«­•?S°oè#ú?€î%Æà,?z'X{m'Ú?ï\I6Ù?~9qO4?a\õ?K
¥ï²r?'[tüÉm0?}.õ¿ñú?ï£÷wV‰á?b¬­yË ?S5t‡'Ç?9AS˜_ÖJ?"›s¦zYŒ?b—dy"ø?ï0G•<á?Ž\håxœ?eŽ€î`â?Wž¿0÷€•?—E=.±.¼?Œ×3Fîà?ï8ƒ)É/½?"\-dÖÞ?X!2ÿØz?c'%¥­Vk?—m‡'¼øÈ?'cPm'å?˜72¶?_U ÒeA?rk>Ëkp‹?mvvdm`S?£‡^¤=F
?Ž§"²hÃD?îÉ|ÊAØ?"€g97=¶?o<|?_dْ
ÏC?¡w|øf=?"B'Up¢AGN4FGL J0224.0-1850¿ËUûñ8ÎÀPËʖ'§]À:ÚlVjoàÀ<•?†'Í@ gšÅ=·F?ûµ1öQo?̩͜çD?ÑŖb,šé@)à¤&?úæîÄnYz¿¡%uŸ-F#¿ÚRÅ؈?çHšÙ4º¿ÉH‡r¥¿á•îê.¤¿ïÿªÛ
}2AGNbcu3FGL J0224.1-1846GALEXASC J022404.29-185029.9?﹞ûÓ?>"äÐÛï?Rï7•¡r?U- k³Ê?~u"šHf?{êh@"›?ï‹Ëbb?`©çY:æ?i–=Î}‹ ?uÃz«ñw?†§˜Bª?‰ÂŠüSÕ?ïºY"ÖG?ŒØ=ðÛ²´?zBqE8؇?|åVchtþ?•ø~FÄð?‡Ô'æ×?ìê»$%E¬?"—­‰¥+?ƒíç|¸ü£?r[ço­èQ?¶,iíéÙÌ?'Òjíõìu?ïqåJ?áùùŽsa?dÈ©o°~?^H8.YU?Šq2Ö¨)?~ñC(èH?îÙZ<•O?£{Ûí¡å‹?»§ÂÆsu?‹Xå\V;M?œåÎvQ2P?žn/#'N-?æ4/?'ÉJõU%?ýæ€î!?}³`']? æôÊ¥|½?|`Ǭ?é½àª,þ?©ˆ¿c¥
c?™£HçG?‡°¤U½ÕA?Æõ^Pî/?©5þ*¢ãAGN4FGL J0224.2+0700¿ê~|¨.ÀH'$cŒ—SÀ:wpoÔ¤2À<F'ŸªTÓ@Rý8$‰¢@êN7›wÀ?Âc\›·V?±áÁ'ýö?îí{ì	©@«ºCf§?À®|ª }¿âÁŠÿ¢âî¿æ'~Ý«—¿ëÙ—Œy ¿Ê
#D}³_¿ïþËí©¼'AGNfsrqPKS 0221+067?ïÔÞèòáù?p÷Ã;'Ä?BÿP'$S!?<Ï/9ýW	?s0¡Š‹("?oÉ6ž,ea?ﺳZ4ÿ¼?€â¼2UÕ?P"ƒ³Ú\µ?\3h*8F?~…2wF°?|¯Xí#|?ïvñòÝ=ï?'cŸõÆƙ?Wʧ¢Ö ?Fꞣ%€?J.E`™?'
X¢ÀI0?ïÀWaCot?[.þïZ?9¥Ð[/?&

¼Yõ?~9òuÃó€?ZÏÚíM«?ïu|×&Þ?°éÌ­Ó?]&P"—ª2?\?­ë7Rq?Žü.2Ÿ8?‹r<(<n¢?ïG°´Ã?šB_Qó]r?X¥GöÁ??c^Ë{ÿ›?•™U`‹"?™0ÿyÊ[?îÐvš¼|?".rŸ¨Óÿ?l#O±V?jCOh¦?¡6Ä"´Sè?'3YåÜ?ï1'ž‰©ž?|ˆÆ@INÜ?U1c›ùú¼?LZÞòK?˜zµüòF"?{•¹ºAGN4FGL J0224.2+1616¿ä±Y÷ ÀDü;OagÀ:y–JYÀfÀ<J¶4‹@²($·Dz@jlBHyì?Á=z^ëÈ»?©ËndÁ˜?ê´¯ÕEAS@xƒÚ?ï;2G¿ÍEäßq¿æóÇb¦ÿ¿á"Þt"ý¿ÞÆlÊS¿àÅFÞ	5AGNbcu3FGL J0224.4+1615NVSS J022411+161500?ï¿6iÒ	U?hAq «?NâYƒLœ?8,ÄF¹"û?| ÎÐ0Ò)?gbJªÍŽ?ïšåšíÆ?}Тy¤ø?ZÒ94]a{?YŽß|+
?…ìvð©=?z"¨÷4M?ïl©Ï¥Lß?|é2u‹,?jͼmý\(?r®!
Ÿ?Ž"ÿLùC?u ðÿEÁ?îùÇ-j`5?r¬æ¬Š ¢?lcz¤e?L_ì¡pT?FmçRù¼?r;äi?ïpĽxŠÅ?}"Á_?a¹_lØ›?RwÕtÊ*ÿ?`xǯ/?{9å7}t?ï'òû#'?'™ÄxIÑ?c†h•Ñž?g8ÅϛžØ?œœÔ…ªƒµ?'G㗵*ÿ?îãÌð"J?‰ôùÃy1²?r~¬¼Ãô?oÿmÍ?žæ¶Ì¾Ë?‡:¬]Ï;?ìé'Vóñn?Ë¢)_?"9{í‰u?mƤ$Þ?¶,9š°Žá?Lü@4AGN4FGL J0224.9+1843?áǾ":ŸÀCn¾H¥‹À:ìxc¾ìÀ<	haQT@wv./"@CEÏíé?Ç`ü" c7?Õ½½eP½@i¬ÿ§ël@¤yÊl˜¿Óp¦{RF¿çF—ɵÁ¿ì¯D]f¿ïÿÿ&¦³?ïÌ"'áÇ0?ìMÃ\á'AGNfsrqTXS 0222+185?ïÞ§kY??ˆ»×ÿRR€?:®ëëFÏk?a;֋¨?nñ+Ԁ?†íͨÝA?練Zœ{?Î_]®gú?cÚ$ÏTÛ?{2lO·J?€£ "[´Ü?†Ù7ƒ?ì‹À[,ÿñ?£Ë¨œ'1g? ²Œ¿øpB?–¯ÇPV?³H¶Ç	»×? Å~«ªß?ïúžU&^J?=aQÆOn«>áúÔåh÷>åÅW=f=?E>À×Á:W?=-7òÃ?ïØEɸÆ0?{«W>MÁ?Fÿ_Èü‰4?Qwkÿÿëb?pý/AìF€?yä"$£æ?ïPüB
õ?Ÿ0"\÷Ñ?mQeÿ£Ž?ˆ–3½Ú‡?'6Utö?—ZًJø?ì
a"	‡?¦kƒ{‡ü1? ·ÔêÚR?˜Có"M€\?·9o÷l…%?¡½.6X³t?ïã°¼Jôp?iS³–K?Y;Iú4?!|×J7?k¼yòа?hûæ¦ùº¨AGN4FGL J0225.1-2604¿Éùj´¸óÀQCÙ+à‹À9xöžWn|À<oKG&/?@f,êįr@ÚÖzËx9?¬¯àš?°ˆ©¡x—?üâqÊG·O@,æyq0¿ÒvÊÍL'¿ã™_÷·\¿æúK '\9¿æ˜§8Ϫ¿ì÷Î8׋¿ïþÊ@*'{AGNbcu3FGL J0225.2-2602PMN J0225-2603?ïò¿)È?h1y•²J;?41ËÚJ»;?63ò£†t?Uu:ͯîi?e/ÐÑú?ïëóÕ5<?kq+»…Í?2¦'±¥oÐ?E€^Qÿ4Þ?a·X'WvÛ?h@~V¼_?ïÃê?pY±Wìr$?U	Àlšõ?U{h3«1?xÚ·¯Kâø?muÓÀó?ïú2…°¥ò?-O¦å?&Ñ 8?~Ÿ2¯?A¡Åd˜«?(Í>UcŽ?ïç
e´¿?p°™ÕÕ?A—Øz8Ú?9}֔†p?d¤\p
U?nÚTIU?ïȕ»=®6?€¾Hsýª?D
w¬Ö?XÚWþ-gÎ?y3sƒ³
ì?~X_Š¥›?ïœ:"5Y?zGÍæԓ?_Ùú×|÷?aàK+bßg?"þò
ŠL¿?wvúþypA?ïñ":u?Kyƒ'Ñþj?>ÈJÁ/Ìd?2ÿ:±TD±?UEy3Vk?Eó)CÔåAGN4FGL J0225.6-4502?ÚÐ%æÞ4ÃÀPNe¾ ºÀ:ËY%5C¯À<niØá®@Ú}¬Þ@ÓÁÛØ‹?ÁÛ«¢Z³U¿`7hÆÕ]?'Ã`Áû@á9|Î\Å?ëÅ3 ïò¿Úˆ€Âˆ%¿èri>‡û¿â?–ƒd£ï¿ë}·PcÅ¢¿å۞¡Á0aAGNbcuPMN J0225-4503?ïð@Nœ»?cßÙwà¡=?9YÁcč?:}Tkr?Y(òcÛU?a'×ÎK?ïèîWW¶?i
þÆwþ©?0Ïψ1ä?=‹>QŸ?d÷Æ{rÈ?f£½pv¨-?ï–þ+6?'{ôDñXÁ?c‹ÓÇè?r˜7T
/b?…]€bÆ£?€4Ö5&3Ž?ïä=ª Ï?HIqQ#¡?6¡_5'n·?\͕ p?hî*×9?G+Ú@r?ïçhþWo?pŒEŠÜ?FÊn3$š?OhçÍ¿ž	?bäf;‡6^?j4¥q'¯??ïÃæFÿ~?{ZÍT©Ê?@a2
\ÊR?PY(B7x?|¶¯
6h?}eýˆ	ù?ïqÅÅqŽ¹?…Ã5,.G–?dQÁQ:è?qˆíȳ
?ŽzT(÷?'Ò÷ÏQå?ﱆz­ñ?fnÜØæ½?QA•ª)g`??ÿ0ØZì]?v.¦Åë?d¸"ühñAGN4FGL J0225.8+1310?•÷ƒu9ÒÀEÑ¢Æi}À:NÈ.›À<Rû15,@ü'Ñ*T'@üÛ`
†Ñ?Ã7²žÎ6Ú?¿0°Ìæøó?úÆ&Nyá@Ú_‡z¿³ùû€Q¿æ(¾e*ý¿ß=ïN×Ôh¿Þ°JJ¦í?¿âqâE"ï¿ïÿm²æAGNbcuNVSS J022551+131046?ïÞûV*·—?`"Ž×êÿ:?CÁUŽy%?6®Wmk1?l>ù~dç?]®Žé%iº?ïËO…¾	?s·W=&C?DˆÃN(¨?OŽ]Û¡ç,?wà¿ÑoQz?q%)Ž{z?ﮗþ
_?r¯ÑùaGD?TÔ¤`Éú?K}Fž5?¿käuM?qÒ£3÷ØW?ï'Öš3¥ý?`U*'¿~²?Xfus­ø?6°ŽÛáß?Œ=…½0Üô?_JûƒÈç°?ï°°j4|?wLáa9—?\ÕýúÒ?S™Lú©<?€9%·í·?tÙæHÝ^?ïfÏB{ƒ7?ŒtFßõ?RØÁ£R?W"ÊW
(§?'*ŽJ?‹rs¾?ïqREТM?€øl¾ê=û?aVe2 óò?a)½òÔ?UÕ5[Ó?~ǀ½–­?îªv/K?jN'ò?nÌÑB'ø?V
êK,3?£kÏû¹?€Ëö?º9AGN4FGL J0226.3-1845¿â{ìo ìÀPª¼£nÀ:¨"7blÝÀ<l¥Ö¾¾@ p®øU@¡Ðº˜ã?ËÇrÅÅFœ?ÉAóU?ù¿g¤T¿@¬äúëï?ïÊBy!T¿àâՂ}ô"¿é\sÔ
2î¿è=•ø$il¿ïþÁ¦þÜê?ïñ"aÎüþAGNbcuPKS 0224-189?ïìѼ¨S?e_9$§'Ë?HÚ¡½ä;?Kbò"ÁK?ZTi!Ô?^¶•¨É7l?ïËÞÎ*M?|—E¥%fà?Qf}yÞ¬^?a:™¾¶iH?u¶ù ó.¦?v§÷Já?ï•Aõæ?}vÛXr´0?qœ@#—Å?xÔµüµˆ?ábxø'°?pŽZ\Öl?ïÜû¨Va?R•8iÞú?<9¡Ò$×?$ÛYÙH6©?o}7(*T‰?QqÇÆ8@1?ïãåYØÛÆ?cƏ"Œ~?QewÖ·?IÁ"#RH?c 
%~Q?_Œ]¨F•?ïŽð3aßÍ?8íŽUœ?W­ŽÌ"¡@?jÀÅγÿ?‰NA@7È?‰S(Àaõ?ïHô÷Ÿoƒ?ˆæ$‰7§?}3dŠ†êµ?»áâòu?)рÑý?}¬¼¹'·?H'ÇÇ?u?FÆqÂ?SÚ°·®²¤?CܲXV/?‹"×ÒV§ì?t;"pÿ‹AGN4FGL J0226.5+0938?×kZLãĜÀGMÔ{í·(À:lôI:ÜÀ<a&õ7O"@<«S«MÌ@Yúb1M€?Æ06(°ù?¾ÑGA_Y?úß;ÒDÜ@"˜ÒtV"¿çØ÷°Õu?èά5}O¿ç›©¿+¤t¿Ê,Æ`¢¿ètõ_èóÊ¿ä{aT¯AGNfsrq3FGL J0226.3+0941NVSS J022634+093843?ïø[Ê?>]üÞ? –8m²—?SIۂ?K…ˆÆb¥?:¢Å§pLñ?ïîâ;Û	?fcR¢³ñ?-@¥Ï9??-÷a¹ß?`ÉÈÃ??cRõð+|~?ïºg#b?lZà£™N?QÆs#ދ?@M9͉?~‡"íØé?jã7ßÓ1?ïï¡¡Xˆ`??ÿ³=ªg?+Ô½±¶^o?£g&}Ó?]B%»ç§c?=é6yUœ?ïòÛä0°f?P'Oc,?1ù}Ë2Ò?+9"iß?V¹§ÊI?Mï¾Õ`?ïÆæ,Ãê?€Ÿõµøk??hÖ/CJ?TtÀˆO&$?z–h"8•Á?~Bè"GÚé?ïiŒFA?€Œtb	?\"Ñó"˜?c¯JãUˆÉ?Œ• çj؝?!ë}^?ïÚ«$[?ZM)­é&ß?>i_ÿ¦nÉ?0+bŽ-ˆ?pÃ×ë߬?X°¤"ÐzÿAGN4FGL J0226.5-4441¿Ûã2¼ìÀP6Þ¹^[À:_Í¥òmÀ<uW¿Úv@ Xûâäç ?ü̏	óžÉ?Áçt†B$?Á0ŸD©RI?ý0 Y;Û@5qß@lØ?Ó_JrÉK¿êС£SV¿¿Ãz
?åH¿ßœ{¡6¿à7#"ú¿äÚséܨAGNbll3FGL J0226.5-4442RBS 0318?ï÷ËPÿT'?<ƒq=|Ž?L¥­Ë–?»rP4å?M	&Ê¿s?:tÃ1X
?ïß)9puD?q±§Vju¸?7l¶@˜‹À?C!T µ^?mé/ÎãŸ?oäÎIš?ì?ﯱڔFÛ?t¹´ãhAø?LO@+."?6oIRìC¨?'N•O`"?tkÂDÑ?'W†?eªÿÆÒ?GñH೶ñ?/ÌI'@Å?‹Ñï蘡?eKÝäû)p?ïíõ4©;?P‰;ù6q?7Tw¦¢àC?+À‡÷Îy(?^@Ú	§Õ?N4‰Æ="?ï¬z`)œ˜?"Xïc²Ma?H	ï
¢Â«?Tەæ§V€?ƒ`Èùø¹Ä?ƒ±Îq )?ïtäîN=?ê<dÙJ>?S®6›ßÐN?VtÒë¤C?(~͆J?"Æޏ¯˜?îµ.ÎR<?"Ìÿ¿Á¶?\æ…aԈd?Lêµä-dc?£ÇXé'
'?"œ"µY1­AGN4FGL J0226.6-0553¿ÓSŽ¿ÃÀMz
í(ŒçÀ:t`§	Ä¥À<—À{†@ÕüT#î@ä;ÜO Ð?»¹J9	6
?'p%_"—?Ôî16ñL@¥$Yт"¿´¡¢¿å0¤ãy·|¿Þ'Ðý‰H¿åÜv"œ;¿âÇîvjÀh¿ä§­­"AGNbcuPMN J0226-0552?ïã<¤1^X?cŠÏßù?;2(»Ùn²?0e¸Û¿á?i]É'¡9?aŠ–@¢?ïãS¦4 ˆ?l™xl7]¨?3ç}Yn-?@•¿¾§é?j/jœ¢q?j6°õÕQ?ï§ìímp
?t%!ƒý‹?[0ãRÿ?býÜ×l?'¢þ{%OB?q8šF®ãG?ï×b>ê]?PÌöõáŠF??!ö8ìJ?"v¢x"á?r\Þ
3uþ?P_—N÷K?ï³w4â,?w‹qˆx\?RUã"æ
?CŠºÌñã?€þq…"1?vQ¾Œ‹Ê¿?ﬣ»AÆ/?…}m.¥±Š?E»LØ	Æw?U{§¾dòû?ƒ{\j­©Œ?ƒá'¤i?ï^¾ç(e?Ag¯‹Ñ3?bìr-ë²Ø?`þ˜ˆ4à?'Ê"Òú'=?€8ÖSêÓë?ï'æo"¿C?o,Þ1…}h?SÐÉá©áb?A«÷žWÀá?ˆÌJÏdµ??m•}ÝPՒAGN4FGL J0226.7+2312?à:Qïz»wÀAS¹bŒ½À:´ƒ*ÂKÀ<aÝ6§[ú@ 6՝@YbÝDê?Â˅úÖJz?—‹|ËW¬º?ÖÏ;üZ"?üà/€ L¿ïRW…øÒå?ïÚî}÷|¤¿ãϱƒ›*"¿äŒé‡îvk¿æãÕAæT]?À‹#õ}›AGNbcuGB6 J0226+2311?ï·1uv'F?qw´O¦ÿ?F¨™Ƌ?1>u>m{?€Ñ¸tË?q´Œ$î!?5ÂH~?ƒö?¤;!?]ӏ2Z??c>¡7]
q?†²&·?€DÝííìö?ï_<o-Eš?€bº¢º<ð?gƒ
v@:6?g‰M–í´ý?'(mË'?}©þÊ(‹B?înÊÛRn?0~äë´:?€µbb´J?a¶³<Þ¦?¡ûÑwJr?}#³w\÷?ïVâÔc-?†ì§pTé?^‡=íew?Pr(ôcgJ?";1£Hìn?…þÆXº7f?îՒěÙm?˜üºé¿Z?m¦âgFÀÄ?vZ'<Ô¢|? ÌeŽn%?—¨ù'"€?îÓbÙð!?ŒTÛZ¡d©?p,Ôiº0û?dŠ «uR? Ä;"/ñU?ŠÌu¸3¥®?ìu;v¬7_?™#6¥~`J?'½v¨èã?€ÍßrrŒ?·¦Æ JÒ?™v%D^ÞñAGN4FGL J0227.2+3928¿á!‹gôËÀ3Áޜ)¦À:Qnf)À<
ÏCŸ'@Ê·Í·-~@ÿëJ?ÄúPþöÅ?£"$à_%Õ?ØzšÛ@
ÈcCqCå¿à«RÿU¿ær»ß>¿X¿ê_«+'U¿âÄC@Çpl¿ïɧ~^ª°¿ïâÁ*ØßAGNfsrq1FGL J0226.0+3922B2 0224+39?ïëQǸ?.>1Ç?+Púž¬å?""´Ç}éÄ?c1é#a?.®Éi†{?ïß½D;Ã?q;eÝ­ï?Bìä]ád?P6ÍsVƓ?kÂ@¸Êì?mÌWí^á
?ïŠ*NÄDy?…úڕüðÆ?f%óx•åp?pç1‰Ik?‡ëïk¡þ\?"_'í"À^?ï·4¤n×?^»™ÊE Ú?S1<@ò?7#ãno"×?™måaÊE?\ÚJˆ•2}?ïï:I§ê?^µ	Èìö?:¥÷Íh:?4nksc t?[.
Øö?]h†ñ?ï–þúï?'À¯Ž÷ŸÌ?TÑ%ïú3˜?h-w<æzõ?‡¦ZOàE®?ÿmÆÈtû?ï4Ê߯	?¼0–x?u)•K"h³?{ú÷ D?">¯P*´?‹­Ëú6_?ï).Ü{/e?måH](²?n÷=ôñD?[ê'U+Î?–ûAM~î0?|º+ߋÒAGN4FGL J0227.3+0201¿É!hì§wÀJgãŸw),À9­ÑI3O¹À<,Y4©@îÞA>c¾?þÈ;4¦?²D
Ëð"??œÃD¹?ì¤ò'Ð(¢@4>=¨W"¿á¢žA-¿àÂñLO¿àŸÍàÉ¿ØKêd7b¿á‡Û+4a1¿Þ`ø=hì(AGNbll3FGL J0227.2+0201RX J0227.2+0201?ïÖ'ï)»]?_TÞ¡u?Eg«ÍQcä?3©¨ƒ+69?r?ûu…?\Oéâ.K?ïÔ¬¸Ù%?sR‰WÚ?C.ÞZoLÙ?LÏ™Àä5?sCÇÓ-W?pëí®Sž?ï[~Vz¾–?É13jæ?g#aö"?cc¢äá^‡?'°¼VV%?€˜1I'	Å?ïMÖÇd?q#fà…?aô©ºÍ?C¯°Ð«P?"'èÀáA?o®Š²ð"?ï'hq@?~œUè{¿?aÃJÈB?R'G˜v?‡^rÒš?{…<=fž‹?ï}Ãêûáã?ŒV
"äZ?Rà•ò'$?bu÷±Eë?ŽN‰60Nã?Š¿¢ž¤; ?kçëÈ?•$kØß?sË{ìC
p?kw‹؟??£<ÙÂW°?"¯ög`?îgÒ¾ª#?Šòw%ô?t†´FE?`nò°Bô¸?¦ò"÷^?ˆ?yYá‡jAGN4FGL J0227.8+2246?눕']q1ÀAvÐâ2À:'3"«CÀ<S¯s²M@ïæÌRT?ÿI-U£ "?Ï0šgó
?Ë›Â߁@kq'úä@kÓ}–á¿è‹ïŒë5n¿Öa/šÍKM¿á‹öþÏ~X¿ßØxýlÒ¼¿æѳ¼ZŽÂ¿ïþû=x†zAGNbcu3FGL J0228.0+2248NVSS J022744+224834?ïñÌ·_?GÙ$t2p?3,ƒ®H¬?"›§ '?W›p–»wÌ?DUÒz<?ïãì%؁·?k>õhŠH'?3~ŠÃ¦6µ?@SûçpA>?i¤	65>?hpÃÏ?ïŸE;Y®ƒ?u§Z½‡Õ¸?]3h7ûݚ?W¸ íß4º?"ˆD*Óóp?sñVm?ï¿R81Ü?Yۏ\þ?Aa
)T
?%ߗ,Ç.?~*ÂÃSè8?Xzê:ɐ?ïèH–û7L?UÕTŒE‡l?AˆðK3?3ù2ÙheÉ?cU-áH?Ræøûßsë?ï¢ÛKZ?ƒuÊ|̀?I	C$Ð,ä?Zü'ÔUǦ?…¸¨ô£ç?ì¨FEÁ?ïI'_‡?‡uGfLí?j$j¿ý¶™?k¨4¿]Ï?"‰&ή Ó?"þýe_Äû?ïW7ù…VZ?wøi6éâ?P§wŒ)G»?AP<('?"‰\iö.?w»žÞSÎAGN4FGL J0228.0-3026?Å¢1BÃ"ÀQ'N;Í5¨À;óÜ܉À<·‹"- Ê@MϹ'0¿@î#yÌ?Í×¼w¯d?µ±-œ"`?çؘ²é̸@óÔyêQÃ?êDXŠÑ ¿Ûw"}~[¿ã*l»>¿â³_þÃ?¿åª""Žö(¿å0´hQøñAGNfsrqPKS 0225-306?ïùÄ'?g¨?3e:öA`?o°¥µŽÊ?ª%@M?F¡lñuƧ?28Sèç2õ?ïå²V©ÚÚ?i_"i˜ŠO?4(Fð–¥=?@ºfW³A?gÈ £:5"?fÅʁCcŽ?ï½[k>E?b©9^[O?N¶µ²Z?=8K»ÆÍè?}{sÉ
k?aU6{,À)?ïàm›íd?N{zžÛ@k?2V}Ä]³×?Šb+N¨?m³ÂŸØ9?Mó†¢f{?ïóJ EÖà?GŽ¾þ/ùï?!,n9d	?痣}!¯?WF1¢m]f?F¦†ÿf´Ù?ï´!/O£×?ƒÎ8"_Ó?Dl<E''G?WזÚˆ¦?°ðo¶"?'Xv{Ý8?Áւ6?tÕ¦×ñ÷/?W#íÚ1?Uû|Uùu?‰y¯O€Ÿ6?st2_M{?ï¤Ux" Â?mO>jí‰Y?C­¶u¼?2¼Rɲ›?…¯ÑˆV!á?mB¬zU\WAGN4FGL J0228.1+8208?èÛ¸¶H­@3뚝¥—ÕÀ:¾R}{UâÀ<\±•+v@je›»1ð@" ß8´?Շ#	ðCÊ?¤k·^%¥+?¬ûŠûF1é@¥CWm¥¿ÖYì x±¿è¿¾ëbº¿ã؊:N¿Ý$þývÑ¿ïÿô╋î¿×·0ÃÂ7AGNbcu3FGL J0228.5+8213WN B0220.3+8153?ïáz­+'÷?qTŠñ^H?BÙBäQ\?@×±K³_‹?iÏ…#ÌÖ?o¾M'e²¤?ïá#Žz¦?qêi—Õ"€?AV%'µ/?QÁ¬÷‡?j|œ?ߑ'?l¥BA0ˆq?ïIìxkL?‹Ë@g?iÊT6âäí?s»ê­5•?"‰1'ß÷?‰Ë =Qä?ïá1Ø.±?J;²ò÷ø!?:&»1½9? š5¯'î?k‰P¯óˆ°?I.©/·¿t?ï¨LJŽø	?Šè*Î·¨?Pµ‡ÁF»?EÛ¼âM_0?ƒêš…V³?Šeh®‡?ï¬INþjÕ?…
´ë­Ù/?PPë
õa&?aF{Y{"?'ãŽÜ"V?'uE<x=î?îzï0¾¨Œ?˜¶×ò'¯?rq' †€?wU—,žð?¦çüS"<?—Ò}Dë;?ﯝ±£÷?høK¬¬ëä?ILãiø ?=݆¶Šæ?'ƒÅl½4Ø?h|{ؾʍAGN4FGL J0228.2-3102¿ï«º0ÀQ"gßã*À;C—'h$­À<Ӂ¶NG@tãÞaIÇ?þùúnƇ?Ï2·¸=žœ?Æ@b†2¼?÷š™ÄaÄ@?þ¯áa{¿ïŬý¤†?ëÊGÅwÄ¿Ô
=¥ýÖ¿êQÎ(í_?µÿjXäG¾¿ï÷£:,K¸AGNbcu3FGL J0228.7-3106PMN J0228-3102?ï•pŠìÙ?®Y΋:q›?VsJ9×·?y0Y¼cÏ?‡ÕšüNØ?«=³†(e?ï¾k•Ð6d?'UÌm‡ê?S3+kº?\«ÅZ–B?|èIšp·?Ä¥¨ü?ï"E§Ì?‰F£c®}?p³aHqÂ;?rý&É"âC?™·À3&í?†ó80?ïm%C¼@?sº nÛ?R"RI…N?E£ÛØ» ?'96^_&™?rÛ45"?ïˆHé¨Ð™?6¸"T·ó?^"Ârhk¼?Y-Ðâ\1?Š-:È>M?ž5æcó*?ïbO^ž,7?"WßÑqh?bi"w4W?p´þ	'ÉC?'hÛÒn«?'I‡ã'©?îvÀ'=?"ºõÑÜ_?{dŒÛfáÀ?}ìÂ˶\?¥'eAÈ ?'/WV_$?î\ÂÂ#&?'¤Ò«29?b%]¥-k?`_úi¥¤'?©ˆxQ?'o'Ç%AGN4FGL J0228.3-5547¿Íp¸
.=fÀL9BÜôb=À8$_Ñ÷®ùÀ;c¤¡4˜Ž@Z4!š¯n@κ'®š³?zùà V?¼âW–>ñ@!±>›A:@€yMHÞ?ë°*Öm_¿ÛœEE"o¿ãZ¡Ëi¿ä!»qZ¶/¿é1ÿ×f.¿ïÿ{uÂ#üAGNfsrq3FGL J0228.3-5545PKS 0226-559?ï€7Ö0"Ý?ƒ°¥´ñZ?qL"eDp?l˜lã£?‡gä0dÎk?~lZÎ?ïÏ¿óö\h?|yªAЅ?Oæ^eè!O?i rÆÛîì?t#:5¾¥X?ví_¦›3?í†Ã§pX?£~"PF¤?¦e<Ü?Ÿ.'ÚwI?¡Œ`nQW¼?—æ³—‹f??⦅qc´?mwU.€%?Q"²¿¥Zå?F*ЛàÜÿ?}C§âï?i¨
ª6͂?ïd¶±`m?‡ãSû>u?yl=‡Z?uApdv_?ŠM‡€?€q[?ïxŒV+A? 3
õ?eoTz¡?${Éö?Œs——Û?™_ƒy]?í;X2hh?¤Ã÷áx€?¤ÖòÍ^å`?/n¾¹4?§sŠ¬Ù!?Ÿ­¹ì]Qc?ï.	ÇýH?Œt°»{?jò¯ÿœ`Ô?a:	÷/¸ß?–àq
l Ñ?Š± g©ãAGN4FGL J0228.5-2234?ç¾Ì¿$²ÀPã8`™ËÀ;i+Õpà=À<ÎÀMb‰b@")øL‹@Ægeiç$?ÓsšvL?ɵ˜RÇ£?õàèÄ3¡@+ˆª&À?ïÿ-½R†`¿à÷
}—"¿à8ÝA90M¿äesâ¥Ò¿éµ_B…¶Ž¿ïôó'H¡AGNbcuNVSS J022832-223350?ï´²UÁí:?t̀F@g?XyfÞ-`?Q[Ê0YFë?¥ö¥µp?qބo7Þ¥?ïÃI•p.?|ÒßAãµ?Tx""»Ç?aa•qðËî?y=Z1Ügf?v‡{ñÛ?ï´'0ƒD?‹•YDÊ_?söèq{?r2ƒ9Í­?š+³Å¼M©?‰¢ ´}?ï—	ÊÓx?cÍ"'T^?^&'®†ö?B«‹è+õ3?†xöÈ!^?bÈÀxS—b?ï•UDފ?'5°	I_,?pÅF"P›O?i:
º¢+¥?˜\ˌfó?Œ_~8í?ï^'ÃMb?"tH¸fÊv?fáY¬°¬?uÀVäo?'k«jiÂ?'
R_ã?îX<V"ÙŽ?—7‡9qI?ƒã ÌØN?`f3dx?¥ƒrb^t?"€R'øT`?îähΆÇk?D¿'™È?l1¡‹g?\5pV‰î?Ÿì²°|/?€ûi¨p8+AGN4FGL J0228.7+6718?ïoߓùǂ@Ã2Ál"À9´€JœÜÀ;€R'KÖ@WFbåÓ@j_ºzº±?À$Ù~6Þ?Ê-_Ÿ!î½@	ýfe§@zâ¾%À?ÎÈ2É«Û¿Ý7‹òç鉿é˜#wÔLô¿æ$Ç_¥'¿êaš#Ø¿ïÿ˒:)ÇAGNfsrq4C +67.05?æ?Ǿùƒ?Àð¡""Å?®ùÂ!˜Ä?¦—d''ô?ÏBp{EÏ ?¼f¾KT½?ãÝF® u}?Å]¡ï‡?®˜ôÜu?®^É!8I?Ôs¾ïûŒ9?Â%&(‡?éñ5DãèP?ªÝBïâ&?¦T–´{¶ô?–½ê¶á‹È?¦@dQÂ?¥öÑoS1ò?èäᴙø?—เÏ$>?¬\¤@œ6?"®¦ü@žO?ÅUPPx?"ª`ôÞû?؝rõž…Å?ÃaKkۓ?Ä¢sR2&ï?´ô\wÕC?ÝSaHfÃ?ÀÑhâ[n*?×±®<­Ÿ$?Ç^Ș	̈?»z(á2ž?¶R{ʽ?à·ãɾzz?Å£Í[¶?á"£>º?µÖ\g"è§?¼œŽ
߈?¦cìó	¬º?Ö«µ5+…ë?³@ËñŸXå?߇O³$7Ë?¥=6²½¯?ÂN²À‡9? Jþnïò£?×QVë…ZÙ?£U¨Ü‹9bMIXED4FGL J0229.5-3644?܌CMeA+ÀPÊW)²€ñÀ9/»£¯À<TPâp£@gHûF‡Ï@´ž¢íÖ2?ªý¼¿õŠ?ÀuýG¾Ûs@ݺӦâ@[¥…`&±¿×GÝyÃ:}¿ãº{&Á¿èkZâ#Ì
¿ê>šš¿ïÿö?ŒÝÉ?ïþüà:è´AGNfsrq3FGL J0229.3-3643PKS 0227-369?ïìL8Š-?z«Xy	÷?Züë6?tޕÕEh~?Kx×1Ý0Ð?VÐS·±‹j?ïëMbM@ê?m8ÎóŽ(?3¤ 󇉤?GÀÃàÑ2?b>xD‡á?héK¿ŽNL?ïèîn¾?"\'^.7
?'	®à?'…5}sé?†òhTâŒP?…":·¶æ?ïü¡uÓc6?#µ€Ú'8?'ZÐøɸ?
¸a¼¢ñg?4"º"tϵ? Y‹4ò"?ïäc0À¬?gÔ¦,Ée{?aqèY‹?dú.Ï]59?TŽ%`?N ‡œW?ïÄ16·?‡ÜÈý¼,?MÑã[¸¸?x±Œ­Š€º?z-(>Ñäœ?€3[qGÅV?î×p·©—?–È!¯a³Í?' 6(,??'¬f@tæç?'q³êÒí?ìPñk/?ïö ‹%b?DqfS1ºD?2Iˆ6
Ý?0­TÀ?LY…|`??mÿEËnAGN4FGL J0230.8+4032¿Ôӆ8Ø}tÀ2€V>Ðö'À9^9ßõž}À;õp­è7@Owbâù4@r9`sÞ?²uFþí|?Áÿ_C}X@
ÔF"ú@´Â%~ê—?íY!…Æ~¿áò•S¹»¿æ­GÌGl¿ç$L£2¿êӆŁ~ñ¿áÉO?ÙAGNfsrq3FGL J0230.8+4032B3 0227+403?ïä2oœx¥?WüÕn«1?P†OlÔ.‹?Fº"°ÂX?cŠh¶¼+ø?R'	­sƒ??ïï&@(¥?f%LÔè¤Ã?.w¹æJ|?=¢þéëéÛ?]ä‰)Œ?c½Šç†€È?ïž3¾2È?€;‰ å?kè,:8"?u\Çú}¦ž?yB.'?wÇSLÁlL?ïì)˜øz?D"áĽ?5†–ü¸?Œ oÆW?a%¥¯f/k?BQ"ŸnÇõ?ïƍ9}¾á?kp.?a$tݯ>Ž?Wfôÿ7't?t'(ƚD?e‰%øI1?ïÇüò*
?ÄÚäŠR-?NfƒUB"£?d/:Ën ?x4¶oƒ¨?É¡qÕ?ïbGqÈ^?…ÜÂW5Ãr?r1û¨ƒ?qGd"?Žd
õ,?ƒ#våØ?ïȉ£<`?dÜ Îmëÿ?MyâÌ?:-ٍõ[G?x©_Î?c3R9Ì"AGN4FGL J0231.2-5754¿êÃøvZ
ŸÀKJGìþ›|À:ˆ׊•ñÀ<›Î ‰ãC@ ÀWH'>?ÿf[~«Ø?¹hgGŒÜr?wôMcS?Á*±"qê(@@œ5UL¿è1}ˆ¿ÔÔBÃI¿áÌoD[y£¿Ú[h¢×0¿áf¢vb¿ÙK¯RiAGNbll3FGL J0230.6-5757PKS 0229-581?ïºk´'R?²ðNŠÿ,X?7Pé8É8?'´ñ쾓G?€ª‹§¼
·?²ñùV=…d?ïß½j´:?miÞ¯.?7:ÜȓÅ?A¶‹;‡?m[žÖ';?jÈÔBS‹ê?ï"è'yÊ$?p–ž_úƒ?Xûñæʕ?Sõ̗1	?‡¦•oW?œ?oMÑ"֜?}†|ö?[—á
A¡&?D–Ö
<?(8¸iÙ?~®)òoâ?Zôm]x—?ïט×
(Ä?hÍî"ÙzŠ?He~dK/ª?;Ta´*Ñ?q&ä¬Ð œ?gd_frÚ?'%p?…ØûÌm'?H	Ö&jˆl?Vò€jezá?†›ßÃ?Gx?"iå1'¬K?ï8ëq—a?=˜î¢*O?bN6[aö?XÁh"Òµ"?–²A'8՞?€p²ùºo?ïKڏê)?yôÜ ©R$?Z‹Æã¢Ô?Fš_m܊•?"ãÅA%)Ô?yY—ŒSSóAGN4FGL J0231.2-4745¿çu}ÒáÀNÑ}àÖo
À9¼<ÛR¡ŽÀ<wš‡Ö"·@W´.o˜@(0 ±»Ï?°sHÞ&wŸ¿—ápa«°a?×·ç"
›õ@LJڪ[¿ßnÑ"2w¿åhªC5ö¿êB€®I¿æhÈ@vÕ¿êæ°£¡Z¿ÍÆRIÎÖAGNfsrqPMN J0231-4746?ïúK˜?H;틾BÉ?6»Æ</õ?Eªmš…;Õ?9à
YH(?/k ™vÇ?ïîýô·øT?gžY;ïf?,8ÑD–ü?AUsíôÖ?^}»Hï?eJ2n¶BÒ?ï™bò¾x÷?€a0ñ?Zn`³Ü?bAӟÑ?†cµƒ›Z®?¿êžìU-?ïù´O¹Œå?- ~e	¾Ë?'aQ@–j?üáÛ£=?CV]ZoE?)Læ@ŠO?ïôÿŒEPË?M´±X2&?D_ˆ•÷R?BMIûã0m?G¢Fã#¶?CÍà¢ÍÒL?ïÇû7ªwt?'Y:"µ‰?@ ‡ó»º?SárJb?yîS->?¶0edê?ïVÎPãûÆ?†›ÁBÿ$?cFx‹]:ö?hëÀFeÎ?'½fÓH¼Ý?…&÷ºÇ'?ïíGÜb–ù?Q0µ2Å?D`7'+u?:ßݐr?[@+àј?K…5•'õbAGN4FGL J0231.8+1322?ïøL8ÀE^Ž`€sXÀ9@¬ï·³`À;úØPŽÍ@?*^ù4µ@F1!àûX?¯¯4'àçÙ?ªØæ`œ¢ã?öÞ¿ù³?@ʚÒÔ£±?åaUðÍ]¿æ܁u¶e'¿ê±]À¥w¿á¾«¡Ú¿ínTqq\d¿ïù>JsAGNfsrq4C +13.14?ïÝî3Nâ?«¨»"xïì?PÍ:ø¥ËÞ?‰Ðº…»P?jtSè(?¥4Ňó¤´?ïê
ámv?iJ³`Ì¿Ó?1{m'®lP?@ü8iÁ)?cÅ9w?fuSÅ?ïUY1ZÒ?ÿOv¢Ù?|é'uæ'?'›·0¤QÊ?Œ5&YYXN?†BtQˆ?ïù¦	Èu?/*±8g_?%ŸÖ"⨿?ê7nK\»?Cÿä>Ñç?*È·îî?ïÒ
Ýtv?§ÒucÓn?RöØýCJu?€&Tù÷X?r;ZóæG?£Ôk$+Òm?ïž½},?'oˆ}*`Æ?C#]͚ï?\ešVŠ}«?|L'ÇAÄX?€hNÆÖu?îâ£'¯=è?–#=bZ>ð?'Š¼@"n?‰{n{×¾x?šf<îõuö?'³ØnjÕ?ïï¥ñ'd?Kí•ý%WÅ?A´¹º)x?6@Þû½…]?WÙÁ¤½öƒ?FG'Ô"AGN4FGL J0232.5-1118¿ØØ&}ÿEÀN½u6
À;FϐÌk~À<³ãcGP@!#T33@?ø~ÃNžÊ?Ô—d54?ÑøXrÇ?ÿªœ"¤?@Î2eWó‡¿ïÓb³S?ïþ!†ù"¿Ò£*g¿Ç¨·aßC¿àMÛÀ…–­¿ä<×â)«JAGNbcuPMN J0232-1120?ï㜦®ñ?^8"3n/ö?;‰Û¿c—§?,¿åîvoI?hò£°Çÿ?\GÅ×ß&K?ïÜË>q¶?qgтä€Y?=b"þøœ-?E«ý6»Gƒ?oˆoá÷?nü¡Ébbâ?ï\Í
ŠG—?…?0ž'?cBšÊh8ä?dgY&Ô?'þ\u8÷?ƒì½ˆ'4>?ï=Š!"û?r±Ý"7ˆl?WBÄÎa.'?=ìã(ÐÑ?–ڏ|6Æ?r=Éño~F?ïÁOsŸy?us
k˜DO?N:¨™¨C?BIÙ¦°?{´ƒ6=ö?t]Œü@Å?ï•ý#=%?‹Æìå¦J?T')oÒV=?h²`Jzšù?‡î'ۑÙ?ˆij"b?ï	Á³?ŒE®"ÊÊ?hÂ0Íaw?l/¯ G&?›Å¡§ˆ"C?Š•£¶k?îF2¶­óæ?Š¢ß‡rL9?a[d;Q,s?U;²Úo?ª‡NÁü\?Š^ÕC+rAGN4FGL J0232.8+2018¿á>Æ»LÀBIöã÷‹½À:S»'ˆÛÀ<Hö~vþd@!TƒêÛ«?üŽÛÐuÏ?¼"'¾¶´ˆ?'8W¾}÷?ɸ%õç?þªÿu@ž×?Þ"@œ¨AÓ?µê!ÇP0¿àÄ=ÝT¿Ô¡÷¡Œ­"¿ÚŠºÄ³¿Ìœþ¨çë6AGNbll3FGL J0232.8+20161ES 0229+200?ïÀݛ&6 ?hGэjN
?F¥°ìNB?5ž÷eÜø)?|ТÇÒ|?fô;ÚÙKR?ï©ÙxŠ]ð?|Àò?Tä®ÍÖµ ?\êrot?'íIH?w¶Æ ?Õs?ïdu)ÅÄ?zòG°˜¹ ?bÅÚ2š•Æ?a¶<¬Ÿ€ò?'Ÿ{^YÍ?y/>¯{Î?î0ëÀád½?àfþ?t~?VÈ/Ï?Vï;EÖö?ªa|
¬E2?'Ô5?ïu/îôÙ ?6ÃiÙXè?[Ûõãµ/A?Jñ¶€úû*?8…tÌð.?}rˆÓ4°5?ï=+7Cí?'«ùf@l?`ËbŠdD?g&8ù¾ö?š~îZ¤Ý?'ПžÊ?îÆ}›ö?Œ:`ܶ:>?n§Ya¿?jJS¨ƒ?¡°ŴՊ?‹&A|.÷%?ëNž`Óªb?˜Öw^?ˆal@?í?rw½"A?ÁE0g7,ù?™~ŸAGN4FGL J0232.9+2608?ß<«¯æÀ?eO Ñ1À:ïj'"À<'Ù\'HC@ ¤¤ä%ƒó?ýí`Á
÷«?ÈÀ˜a
[ù?·è>˜A*?îï
'ær@=äÉás?î:¦>Ê.¿•+Êz`ª?ÁéýŠ.í~¿àœ~á\{׿ßµQ†'¿áhÖÏ)žAGNbll3FGL J0232.9+2606B2 0230+25?ïÚµ`Ó,?jì
ø˜°?1)`
j?žc(Äã?q'¿_Ñ̼?j81"ûk:?ï¬è\ä÷?|ìߊ<K	?S§wÙx}O?Vs¤
x%?'ƒÖí?¼Œ?y´¨¢ ÕÑ?ï‰ÙÙÅa?pï
›÷PZ?Zߺ¡ºB?Bˆ:ëMõ?Š-IJ—¯n?p2"IJ+/?îÛ®nÓS?yþæZÖz÷?pN'mŒ?Sf2Ðëø? ;FûWÍ?xÿÝ=+ÞA?ïµk&""L?rŠÈ²j,»?Aã"H?1z)ý À?‡/ÖWž?r1ýÌɚ²?ïéTlê?–¢V~'Rs?f;¢ñìr?nÖ<õ@>Î?›ÔŽ!F?"âò¸u¦?ï2ñeC·Ì?' Û8ë™ð?b"çÄ}|?U®Æ¥?—]'üHDÐ?3{ÿ1?í)²Á]ØÎ?"ì̇ݣ?~^2‹é'?l—W•«1ù?´ÌˆÁE3?"—ù´ËôíAGN4FGL J0233.0+3740?îñá½'pæÀ4ñÁç–|¯À:ç±m˵vÀ<£¦Ç…ò@˜AÖd%D@‰cՒn?Ábǵá£É?ƒ:5ØeC?Ãþv½÷qç@'3úý?ïüp(‡Ç?"AØp!¯¿äÎZÁlœ`¿âü¯ég7¿ÜXRݦ)¿ÝDÉޅÜÎAGNbcuNVSS J023308+374201?ïÙQî+º?'Ë`Ê:Œ?h†Òc¯è¿?'9×!‡p?\Ç·¼}Êà?bƊÄ渪?ïåÏ¢Àï?eži-/Sü?+}ízûÔ>?7mó7f?hx~b¤Ä?dΡÍÓ?ÌC?{å7\w¢?ZbͶöÜt?d\½ÛÚ?‡Eb˜xÌ?y´~ãûÄ?ïÓy)À u?T"‹È"z?EÌ
ܼ?(b-=ÀÑ?s‰èf#R?SÉA&¹ÆÁ?ïڋÀ?v*©î©~?Z"厒?t‡'>‡(?hmæY†7?\Í_ÎU¼?ï´¯,±l}?€ÝšÂ9ÿ?B7¼¯c?Wõ@1g?³ÁP&dí?£b¾Ž¸?ïUəI±?ƒ\‡[þªR?a\'t>es?f¢@¥Ã8Æ?"Gë7W@?'\0ä²Z?ïƎ' ?q̘™ôCB?]Í®Rp¾?I­$‹´V?ŒT¦›@Õâ?q¼±W‡AGN4FGL J0233.5+0654?ç‡Y'à´ÀGøAþ¨,À9Ì$$¢v¸À<8 ŸGX"@þL'¸€@®ÓØYÈÉ?±.Ù\R;¿}éHi·dí?ljÂáçf@
GU6hG?ÄÜNŠ|›1¿ã>åD'׿äÉ)¿—>¿éú)Çy¦µ¿Ñ°Zü$ÿ¿Üw¹à`þHAGNbcu3FGL J0232.6+0646TXS 0230+067?ïØ8}õÏ%?Š»ÿŽeë?0ëÙ)å?5'AZæ¿?rã'0£œ·?Š~ìÅ?ï瞟4Z?hý¥Árâ?0ÿâ'lËn??ºÌÃÌ?fAd"ÆM"?eÂA˜ ©¶?ï;»ÁÊ?"Ê‹·«=á?V»L"?]³ËÉítb?—2·­îʪ?"Ãœª÷ä?ï瑮,'t?H¥Â&rc´?/UéKŽW?ÞE€'?fxó:+–M?Gx0þVbº?ï}£0
"²?"s6쵧?H{]-]K?ID,ts?~dm?"ÜáÎÙÅÃ?ï¬p—tm?ƒ/ËL—ˆ??l¶?NÂ[£X?ƒäe,n	Ö?'Y…¦tRË?îoÒ¶Ï=? S"!®,?aå.i?Yۓs–£ç?§ò
µ?ÜG? O›{â?ï»ýSAO?hwœö#À?FöªX×i›?9¹f6Xۖ?"@þ"?gu5)56AGN4FGL J0233.9+8041?±.@VZ M@2­‹`ñ²_À;X¯ð3íÀ<Ïoì÷å@"Ď_|½?ô'ß(#½?ÒÜëû?ÐÄ C?ùƒš¤["{@ªM¤x›?ïù9r•T¿èº'S¸¿ïbË#/°?ë©b>älQ¿à°Ã¢ÆO?Àš2›³¥4AGNbcu1RXS J023428.6+804341?ï«lLë|?}{s+°X?OøÙ^/?F%&wÂM?ƒ@ÒS~?|uõȕÛ?ïiŽ•žQ?–Q}öûÊf?jÍôëPý¾?…Wk?ŸDÌN?'Ä䨰?î' 8¢?šUyM+©g?u"¢Ö¤|û?{*fR¾Ã?ªÛ‹¢þÀ?™±è×-é?ïF·Òó5?†L!ê×?hVȨi¯á?b-K\³«Ý?šìOê'h?……¢*‡Ÿ?ïr"'®Uú?÷ààß?_=uëåLé?XÜpo-ÿ?ÇI/gÚ?Œ(·»4ø?î'üdPGÒ?µö'nkÞï?xÝ-‹]$¡?ˆ†&£—o)?ªd"
•Å?µzHá|N‰?퓕KV?¨?¡1îƎó?{£®ÎèŽ}?1‡«À@­?±©ºGØ? gìÈF©}?ìµ<C8u#?¨«lä["
?‡d¶èÐ]?Ù
ÊY?·iší9{b?§gíü§˜ÑAGN4FGL J0234.3-0628?³fviX­ÀM?À	oëÀ:š±§­YÀ<~Ûúg9Ë@ f'úÅÙi?ýN$Öyù?Á´-¼åN?±6ªy?ìÂ7åÒ?úÕAX:?ÐÑ`ûmt"?É
É݄*¿×—?!S¿Ûü›KŽ¿ÜÅ%Ä4ͽ¿éŠýtŠkAGNbll3FGL J0234.2-0629SDSS J023410.30-062825.7?ïÓ^JI`'?`H"•:8²?=mkðÒî½?(žÜZ•?tz.2f?_UsV'?¯?ïÃŌ3!?zƒ±*?Pî«
'?U~ác?y᏾)Å?v•/@a
?ï"ÞÒïâ¸?r¼¬jjû¡?a6óuBÎ?\Gƒ½±F?Š}{ÓKq?pK9·Î7W?î]öƁ?}ï×j"Ü?zlT4à/t?[îA²ê\?¦Ó	
Tì?{pŒ/ºƒ?ï¦üè6y?s1!-GÆô?R´Þ? 1e?Bäõ?ƒê*ǹº?rS4fÙ7È?ïH$¼¢Þ?"i¥5.5?cƒ(¾æV?j7íí£,?"‹N _?'Žôí*ÏÝ?ï:ÒSÊW}?~œÑh…(?g~8À¿æô?b‹à÷€<?•µîq´¹‹?|ÌþI<L?ì,ˆð»$À?•-@‹þ~à?‹@Kl…Î?uBg¬Ø'Ù?»3¯¦	G?"†*;žÚAGN4FGL J0235.6-2939?æI¢O9"ÀPÀØì•ÀÀ; ìy:~À<Ä(Ï,"ž@þ™&F|@~¡ñ?¸''™z¿¼'å XO¢@9µ/ê©@5¬(½c¿ÌéìjÕ·¿é8ÝA90M¿åÆ×ÀEÕͿب'n¯¶¿á ˜%ü¿¥ 6@Ù¹ðAGNbllPHL 1389?ïÎaDh¶?ˆ	 ÂDî?CI!V ®¸?\.û©û¯Ã?vf9ÀJa?…Wêx|?ïÎ
Ì%¡¿?y>¥!K ?IÎxN‹˜Ž?Qâ­lé?uÀÊÚ]é?uÎ;€Ðp?ï5S›ªã:?‹å~1yý?X¨6ñ%î?DÇO.‡²j?—Ë	»Ø?‹Åb†n)å?ïº@l&?fº‹é8?Gя¢3ÝF?3WïCH[R?å˜×óÊ?fG#Öúó.?ïˆû,¼å?áDðÜ?Z¤N%ÂOM?Yl­Èè¡?Šl«Ðêï?€™=_N?м¤?õ›À:?T%á"n²F?`þ µÛU?Œ'A™C²?Ž¦/—+Ý?ˆ
Œ1?•å÷ùÈÅ?k[&Yj†Z?p´/Gm?¥Å¾ì?"~K–s¢Ï?îì©ÇFë?‹'ؽ÷f?h¼@ŸwÀ?^C5ùzïy?ŸSC›v˜­?‹qC@ì'AGN4FGL J0236.8-6136?ì…2Òú]ÀI¥`Z³«À9&u =)À<\·ã0¼`@âô©	Ï@ž~Û¨1ã?¥3£E"à?¢gÿÚ$?ôŒ]VlG@³O؀Š¿Ú{?¼X‹\¿à.¾#¼«¿çy!¿mh¹¿á ð¥ïé2¿è%ìIiÖ¿çêªcyAGNfsrq3FGL J0236.7-6136PKS 0235-618?ïö7XÉx?]"¶ë/?dË=P?$¹½F8ä?Qʄ£qÏ?[BއrÝ?ïï"µ¯$?dŸ¿¤vf—?*³M|>ڃ?<póI5?]ªlýß?bFœ
돫?ï°¬žë#`?{ÂجÒÏý?SE}³Ã,?`'Ïàz?l("oò?zßê#Q?ïÿx»Ó€E>ý_adsòì>âòÜ1ë">ÓÆ|ºTÃÊ?
PÆ-0Å>û.b±€
?ïíòqw®?aŠˆé¢ãF?)"ºeS?'d
ì&Ǹ?`tRÊn"?`iü˨—‡?ïւè4?xÚEL¶Í?6ëDëùáÖ?K\QÑ#¥?sO× '¸«?w©‹¦P/?ïrdP?…ø
×äã?ZUÝz—'X?WÔ4& ›Ä? [•ò?…ŸÁ Ó&‡?ïþºÅ…¨?³Â"û8•>øe{j®>ñcØx­ä?!Gü…`™?C¿ìêLAGN4FGL J0237.1-0714¿î‡DæA›‰ÀMY>_· À;«ïÌñÀ<×µ?èM\@!ÁŠN"
?ú-½qåö?ՔŒ¿kG?È`:Ó:¥?ó.a«ì@ÁÞtj
5?áîÜ÷½;_¿ËK|Öt+?Ö6¾£>^
?Ú7D9ë´¿ß•ë/³L¿Ù±ž6ò…AGNbcuSDSS J023700.77-071307.3?ïá*'OÎI?[ӌ›œW?<R‹ðVg?($ýðñF?kK*à¦5ñ?Zq‰8Ý?ïÄ;—
€Ð?xÅÑm‰Ýò?O+\}AÒ?Wt½§úà"?yüÈÔùί?tÁ'GÝ?ïdy½¶?'šn‡^?b»~NÅ?gQæ ãª?'mÍ(‹f?\']Ð@?ï-ƒ]¶?äÉÿwá?O¢ûb‰	(?=þKMú4?™R‡¸ûÇ}?¦J.…Ð?ïʝèit?iEc_‡¹?HðúG's?;o©èàº?w'þë†?g²O|†6?ï}5à.ð?s©KçÄ?U¹&^VB?f´lû¡6Ÿ?ûc?Û?Œ¢5rÉ8R?ï	$H´¥?ŠU
SˆA?eîϊNƒ?d«ëUÎéˆ?œÁ~hzc?‰ØÖ¬…À°?íÞbubz?œÎý
?`½:ʊ‰þ?_®+ ??°‰‹kn?œT*·+ÜAGN4FGL J0237.3+2000¿îQm=p"þÀB,{5*"8À:úK‡½ÏÀ<x篷é@ [' NT@úŸ{Zê1?Ä×	&Db[¿v"ÞÖ¥ï?ªq)Ò?ÿÙ¨'{ïæ¿ê†_ô‡Q?¤¥b5æR¿æ;Z^›@ä¿ÚOõ^f¿ía@"ð'?ãT|YóAGNbllNVSS J023720+200033?ï2¶%#?ÕǥϦ?`vá¸1)W?U1c;ê?—š_á=Ò[?Œ]›K&m?ï£Ó2'֚?€wUªŠ
c?VFqn¤BÖ?W°EƵf?"BeCf]2?~4˜¡î›?îΞôU?"Ç9Ö^¤?u*➜•ÿ?sß@? yc€Cas?'Ú¯£&$?ï*šºÎ?
?v.Öðx¶¾?d­8õji?I·º%ßg?˜…Xrr?u`sHO6¸?îšýúÂ("?•\Àl¹‰?m2l!…óŠ?cVúB);?¤|ù"šÆ?œœÇ€Å~?îöJ›Éc{?—eɨ˜¹?fIt7Ê?p‰†2%ði?žte˜¾±?•ãU÷ɛ?íú<Qiÿù? —hžÇMS?y¾±‰UûÉ?{]kº¾ûN?­$dºôðô?ž¤c§8K?ín<,Åʔ?"h£ÏÊÐk?{äe¦À!,?lYö:N…?²ÏØ?e©O?"ÊG,&‰AGN4FGL J0237.6-3602¿æèïêÖo…ÀPq¬ÄÀ: mÉ17À<}Ötì;'@ ]€‰¨4è?ü²›É?¾a"ðg‡?¦_
ã™ÿ?ér\©NBƒ@
'r—Í?êíý¬i¿æ¯2BGx:¿¹ÐÔÄ=F¿Ü®}†¸–¿äú•þ¦~?M/]»œúAGNbll3FGL J0237.5-3603RBS 0334?ïúO»ÃÔÅ?2œÀ!ß?6?"Ÿ±vÑ?¿ìIepw?D<¼íÅ?1"J°^º?ïáãÀe»?n‰ˆƒ22?6|pJ_.˜?Aþf¸Ç?kL±ñî‡?kªçkÔÐT?ïÄÍo½…»?`ztgkž?K°²*NqA?5M!ŒT>Ž?z#1×Â4ö?_…/ß~›µ?賓­A?`[h3U¤ñ?@d›C^ºô?%Nž'MÚq?"'ØáãG?`	î;ívý?ïõp@@8?Bo,µ³™Ç?'h³m4G?hƒøphŠ?R;'é)ag?@ш½÷¬
?ï­Oo¦–?"ƒˆ}jùn?Eò<ËÁ	ò?RB~⬅¡?ƒMmÉì"?ƒRæÖt?ïš^ò\\?u¯?­Y/?T"؝?IÝ~l§)?†úõÈý1?u'ŒŸ×¿y?ï´Dãb?Íeòú¾5?Rç> t3>?C$gB÷?œ»z¡'?[§'øâøAGN4FGL J0237.6+0923?s>ŒoJÀF¨ÁTɅðÀ:XœóÀ<U¹}d¯­@Ij¸…˜@ù½ƒƒ­Ÿ?ÌÆôE·š6?ÆF‹?8Ð?üÙíçχ'@…Öf(¨ì¿£Mʟ\7u¿æ‡uÀ –ù¿á¡Ü>ñ§¿ãB–³5L¿èÁYAºµ¿ï÷yHÁ9òAGNbcuOD 58?ïž%šnV?¢ÓWȗH?fÚñô;¶?x>h'·¶(?Šaºß??žºœÐY?ïÁ®Ú}?r>¯[Ù_Ï?K}mÞKR0?MéR_{݀?{¹`ïna?pb až{?ïŒìR	s?~"Zx¿í?d˜XS¹"?pÂ
º?‡Õ.ÆÜ?yÐ4Ùnx?ïYç[³é?fù¾.»µ'?_°èbÐêÊ?;1õ«Wâ?'ÈÖî4?fêzVæ?îɼ'¦í?§""rêãv?}`=S?…{ioê¥y?Ÿh£éâG?¢ºe2'Y?ï<‰£'P¨?'T¼½,"(?^¡fåå¿?eoÖñv¡Þ?–"µî?'
`Q¹?ï+¯¾œA?‰û˜Â>?lZ«åþúU?l֎ˆi©?–þ²¹Uj£?‡	î®Xt_?îK"ù`mm?…Q÷¼U?p[CUfÐ?XìÀsÕ:1?©;Xà+?"ãlæ! {AGN4FGL J0237.7+0206?Ӊßc
§šÀI'•þÚfÀ;5‰+L"À<±&9O¬æ@µY5¦U@—?úÁҞ?ϵ8ªå?º=»aëW|?íUӌÚn?ÿ"Üj ¿ïÿMR™*?ïüˆFŠþÌ¿êó_s-F¿—Oé¢E¬¿å©Ÿ÷Ó¿ïÿú Âî'AGNrdgPKS 0235+017?ïÑv䧣·?l®e²M ð?:·ã_w-?1
>ë[EI?u™qIc?kš÷
 †?ïѨªÈ?tõE{…–?GOïth?V4çÃg+/?tBÝ0'?qj¨¨§Û?ïHÀ"ƒý?†¯'0¬¬W?g'¡zˆ
<?mPŽZ•?"õ™aÊÒ?…:î.¸-?ï'À&v6h?j?:Ã?nL?dhĪ€Ð?LG'⇞k?†5ÅCG{µ?gÐƧ'?ï·#†~?x)Ûæ"$±?L.Hµ.'È?I¦'ã¾#ñ?€t9Ëñ5-?vÚqë»Ñ?ïnëApÒj?';BÀ&È­?Z¥ýb9X®?m¾j¦n<?x7õàC?\ ±3:Ö?îÿø/:?Šï¤6W_J?q‰IÂM6N?uõ"«
Èà?›ž§ª¼G=?ˆaÀJ™'?ïÔ0ï?":-7)?uӈW™ÆB?h"XmVÊ?™°š"S â?'~1§Î€ÎAGN4FGL J0237.8+2848?ÎêYãÔ®ÌÀ<†E^®âÀ6âб§­À;<éõÒ@÷÷ÈÎæ@«9²©5?‹æ©¸ËŽ?¶NêÆÝÊ@(=îVŠPP@!%U¬ÿi¿Î¾üÀ'a¿àkÀ]RÁn¿åß:Wꢡ¿äp°×£Àd¿è6c¿Bµ¿í(/~ȲâAGNFSRQ3FGL J0237.9+28484C +28.07?ïÁÀza£'?xÄ,D'•?K¬«‰Lº?GËnG¹¼?{ª-BßÊÀ?w¸¼¡:à—?ï'ÉÖo°4?"¾›rt?]¬ìvz™?v^?üD^ª?‡×ìÅÎqa?'ÇØë?ÞÐ?ïmªh?üS5!Ã÷?‰©þió{È?Ž¡A â¢È?v·0[?|쌰§þ?ïíøÄ!'‡?T·D$'T?AúÚòxF?=^7ŽÑ°]?[
nŒÞG?N`<›u+?ï¹ ac6?}\¶®å ?Iñè²'?DGŸ®'?€ÍÓqOx?|Œ'?-î?ï‡Y٘Á?¥.ùfىç?yàãÈîB?"x#"%+?—7
SÚO?¡üR·¸¥?ïƒêu µÏ?ŽûC0@	'?'r‡Ê¢Æ?‰HÑ+ám3?zçàsM¢œ?ùÇ[L?ïÒà½oŒ«?o6÷<ÔÈø?SGâÆÌì!?R'Ç{žkÄ?q½¨£"ó?j‡ËÕ¿,AGN4FGL J0238.1-3905¿ï¡m$_uÀP2ñVIÀ:B´½âN>À<Š7Âäì@Ój™üÀÛ?þÛ¬´('?º9@‡Y¦?ªŸbM–Ñ?ò'í"Ó8ø@!O0ï?ÛàÈâÝZd¿Þ"›Ãjxo¿áxkì¸$Ÿ¿ÙáN¹÷¿ånß{ûùá¿Ñ顙Ã5AGNbll3FGL J0238.3-39041RXS J023800.5-390505?ïøÿ"_?6صÅëx\?‹‰=-kt?"YƒÍœ?H@Üð?4¤U":?ïèÏãqn?ifÐ\1Ì?0<ñºzx?>"\õüÿ?eڑë1e?f­ñ¶­Mñ?ïëáù7?nmÿlœ2i?PNEvPà?TièdúsÙ?zb†Kuט?lWG²—§‡?ïÎ^kVvj?S»Ì}QN?B2Ìý?%†Í|@C'?vˆƒ.¹ ?RDÏÿ»nL?ïòýk%<û?E4'q|­Ï?0­¸5t'?æqâu±?UÙ»ÿ'JZ?C"$Fçw?︮ ‰D?ƒ‰_¦_ûë?CŽ‰•üü?VŒ'Aà
ô?€Â«o‡²É?'B'Lwj®?ï¡5I/kJ?sJ¥"žbú?Wܚ"h?I7ÇG© ù?"Ò=¯J÷C?qýىœ!?ïy_å˜Ë"?r‡¥7žÞ?V\÷ÖJ?Bp¦XBí?Žåûèg?qZ9£5òAGN4FGL J0238.2+1531?îQ@h ÙÀD˜²é̸À:n­\ÄýÀ;ìg
ÑZ@)âøc!@n<c?Ê)^H4Í?Âá
6u?ø¢ê`[Šj@rK¡éõ'¿èe‰&"Ï¿Ýä8Ž¼ÆÅ¿ä
€¡{k¿ãUÌ»/¿í;	Uê`¿äËÀ}‰ÁAGNbcuCRATES J023819+153323?ïâ6}Õ2?_ÿA¶#(&?B˜+®pjÀ?:Ñ:é"oG?i#ànš?\ûŸí%?ïä'ýì?ls Rœ¸?2S÷éNb?@êùa Î³?i¥ð3 û?i³Õ´lΞ?îãÔ©~?"«ÿ0?}ñŒ^m¨?Ê=grâ—?œ	Zïý¹?'Ðeÿ%t
?ï³M
5-ð?_w#¬é;È?C´ÍgRzÆ?)馎/Ç
?ñoÚ["=?^1$†µ?ïÏÁ$7?n¨½že—?V
pËýÁ?R8¼Êú!]?rù/_&?iì­ä9…õ?牢燰…?ƒ¯_S¢"?D^°
<?S¸?ôx©?…X^&Vþ?Å×ZWU?î­šh²­?œ«K垺?'gÏú)(?…7ÊH?«$Œg²	á?šÕŸ}?ï9¯§U¢|?|Y:É÷z¶?V,yП/?FÔUÛ)Ñ`?—gC'¢w?{~F2‰AGN4FGL J0238.4-3116¿ïÂr·¤êÀP•gÊêt~À9/f±%À;êmÀÍ»	@­ÙY"0,?ý0qLsv?§×Q
3µ¿kä#ü'?Ê]ÜT)@È/¨d7¸¿Ò¿º•'£Ü¿Ü.ò£¡¿Ü!HO$+¿Ú¤Š£ÝjT¿ßß­Ácã¿Å¡gÄ4w×AGNbll3FGL J0238.4-31171RXS J023832.6-311658?ïôœô[ËÈ?HÆJ-{» ?!v V-Þ?UßVÿ)?T—S`%·Ñ?F¿/¬ºÏ?ïï\ôøô?g2ÅjNó™?*mD\ù­?<"ì\$?]ømÅn?d—
^§?j¤AF?"
+ŽÄ?Xǁ•ÎÌ?aÒd~iCd?Šúµ(Æfº?ƒÁf#ŒØY?"h`ͱ?aîþàL.Í?3éÄèØý´??ÕJ^×c?€@Áîo…?av‹š£êá?ïæªÈ)>?]Å)fìù1?4 Ê)
ª?+¶NÒ2võ?fÑÙèóUÄ?[˜sguþ?ïÉPyr»<?ƒ=-n
?9_ïzÅH?Pȼ5¿™L?yÁÄf¼ï?'`X.dW?ï2p¦ð?‹õE¾…t9?_§"Zwß!?dû'FœQ?—·"gã|?ŠÓ ½©ˆ?ïkƒa§mu?zò⚛J"?ERw™?5¿gÛ?'æóCÍíÜ?zSn>…w}AGN4FGL J0238.6+1637?¬¾\ÀC}'Ó"À7¤l[ríÀ:þm'JÈ@(ôï֒@·{|x £?f÷'`¹v?·‰.'dœ@(æOTÑé@!#…k9_¿Àòèn¿Ý;'¢‡(ÿ¿ã7GpxŽ¿âVûŸs"a¿çñ=Å]m¿çÇFê AGNBLL3FGL J0238.6+1636PKS 0235+164?ïÙ§ùÙ E?gk˜C÷X?A#¥»¥"?<ô£=9€?q¡|—vC?e*øys©?ï¢Y#\Ñg?€L¸â¬?]wxÂu7?tb²ižZ?ƒºÕaòg?‹atT´¹æ?îÌïiÚº ?™,z›øO¥?'Ó>Ç_&?'8™#§úÛ?•Ï?…á\Ð?"ט`g&ˆ?ïـ0UÍ?fWØÓÇ
?CcíªÕ??˜PT:n®?pӇ=ÙÊ?c™ÿ!Ó?﹞lg1h?qOj«¯?P‡ÒŠ…+?M¨KÕ`þ>?Õ=±&Ù?oøù<H°ö?ïÜaa¼*?£#CÅàF?mS'û}'á?'@!Þ@|?˜Úšˆ!º?¡ðG¤÷t?î½vn#ý"?›ßªoᬆ?‰0"	¡XD?Œãbw"?›¸èº=`?—TªÓÝö?ï™rîÆ-?€!"Þüž?Uݺ¬Hþ¹?R'­d¥7²?†ç	æh?~ÓÞ<AGN4FGL J0238.7+2555?í_#=>FÀ>üú½ ßßÀ;ÙÛ©¢À<…'e²@!!þ}sô?ÿ¤óÕORN?»äY€¿¤•Às"?ãI›árv@üó€À¯³?ïþvÞ-È:¿ëÃ<?ÌHÿä>>I竿䊗hfñ§¿ÏYm3࿦K_
7ÎAGNbll3FGL J0239.0+2555NVSS J023853+255407?ïOµ­K},?žÜÎ!¶‰?EkIØk…?DäÐ›ÄG?•]ð+Á§?žTyþy?ï‹
‰DP¬?‡[.
:§­?`õÂ)§¹ƒ?jAÂ>¿³~?ˆÿ-²rº?ƒg³w?îÙÕú
?'LԬێÞ?bL~_ã´«?dd©[d¬?¡=Øuþ ?'å܇7¾Ê?îûïuKå?ƒç"}÷.M?Y©Çéì?EÈHë?žç€ýø[?"
$ èû?î¼S?ž"Ý¢Dÿ]?S.­A¶?IOá¹îñÙ?£¥ì§øEæ?žBRØ6"Ä?îÛåû-C–? uêQ?i³ï-…®?tL«Üg¡†? ¦hKMCE?ži$£ü´?í"Ddw½–?žÝTIýPØ?fZ
=Yj"?cš› Ò—k?²³p‰|?ž¨Òz>h#?ì<ËDXìÎ?¥=þ?Tù?uU¬£mH$?n¬ziùþê?¼ÄK(úÔ?¥²6ÝMæAGN4FGL J0239.5+1326¿áFòÄÇßlÀDØ΢âaÀ:ú–xHÀ<là‡"´@û-8¦?ÿâZµX<?Ñ´`YÜë(?Ç#–=áã?óV]Ú¦ª@žÃmþ`C?íñ'QS…¿în16ñL?Æ2ØÅS†»¿áô²YƒÿÔ¿ïÿæ¦Sf?ïþùÛ"ÐåAGNbcu3FGL J0239.4+1326GB6 J0239+1327?ïßÙðÝßU?m·]?U''E<íÁ?^¬2Ÿ£Â'?edû…""?bøÿ`íÞo?ïÇíãPzt?{´-óÂÖ?MT7´±Þ¡?ZàÁs—Å6?x^‡j…'?wÀÂ`3Ý­?îÌ3¯ÚΘ?—'£Ú?~+Bº2½?"À;ÞK~?žî¹YóÿP?"ŠfŒã?ïÄã²É?`µøäÞ2?+©ÍÐú>?|¸+*‹?}!ÀvÀL?`mƒBjŠÅ?ïÆ]ˆyê?€EÏðQ7?eF™–i?seoFç÷r?rS€‹ŠF?uAÄÈ}Ñø?ïraUý¯æ?'É€8ùZ?VR<æÍÃZ?jc•á\?N±q…1
?Z‹ñù°?îk8ªÕ?Ÿp뺩¦?';	·SÙ?†.ÄW–?ª
Š–¶½?Êôf‹þ?ïC§ç‡…'?€Œ_/f#?<Qªdnp?2déøU;L?—¼f8žK?€t-TÂåAGN4FGL J0239.5-1353¿áúK±6÷ÁÀNÃ3ÁÎl	À;sýþžÀ<we'+@¦œ%.@œløPß?Ƭڝwö¿« 8Bf­?ã#û½{ 2@Ý»´MпÓ
e@¡†¿ë䩘^\¿æÏ€Ü3r¿âf="†¿ïL_ŸLáÛ¿îµ{aöDAGNbcuCRATES J023939.13-135409.6?ïó™Y¾ç?PÅx¢''4??Ó>
§É?6Ö<½£?PØ~Î;ˆ©?KÄûÂ?ïÒ[­ƒd?y¸ø¼5A?J'­ÕW'?Z:Õ1…?s÷M©'?t%	=ëš?ï[¯ÛPY?…_õÖRÔÜ?j¥Eª7µ?qR‰
½_¨?'5[ì	ßð?'ÉãBjí¹?ïߪ
2¼s?Q"ñïŽ?FH›BÞ(?3´uî?jÃôÔ+OŠ?Nõ‹p?ï嬐¨j~?cMØÞ¥}®?U-KHmùù?QÞ¨b!l¾?_y"q»Éå?][¬"?ïvÿ<zs}?"¡*éäP?^pHØ+
Á?poԜ¢?Žr'шß?'Šãu4?îÐYŽÅ3?^"¦cÙ#?o™\à'1ä?qÍéaÜ0?¡™¤ˆ3?›D~/?ï›ZI«"a?ru;\÷£¢?b²džì÷?X3´sšL?"|ÔoŒ"?pi<BO
AGN4FGL J0239.7+0415¿íҚðfÛÀH'øã¬cÀ9ƒÇhß½jÀ<4Dé>›@~UñN6@ô±$Йá?±Š*!!ôÙ?°ÃʀÓ`K?ö‡‰	ÿ]@_Ÿ —$I¿ÄE¤¤å}¿èTKç_J¿éó¦öyn¿æûÖƒó?¿ïþ©žttÇ¿ïßÂð|AGNfsrqPKS 0237+040?ïøüÒµ*?h$âŗW?2ex"Ž?HÕòô@×î?FŸÙ°P6o?bF9Q…°»?ïä‰Y°u~?vK$#raL?6åñNóG?PŽ`Ãkç?h™è(â?rÙ롕¼?ï´íÖeZ€?x"ê¬å?_-
©È'?gæûJ"J·?}½ÒW'
ž?tKÛàâ=?ïø dµ%?3!;2±ƒ?+ùëóUÖ?]yïEQÔ?HŸ¨šôþ'?0՛Ák ú?ïö±¬NÁÉ?N1%þÝÝ?4Üí¡«2ó?3"0—¢?JÊØ젛?HǍZ»?ﰇί¿»?ˆ…´ûØ{?G¡®Áe8?Y®UOR!°?'cûæâjø?‡qÅéNzÇ?ï…éÿ7®?€àÙFrH$?e'¼°¨Á?iÔÃvÄÐÓ?‰;'WAø?~,p"Ø?ïéKÍÖ.˜?Uܖf"Ôq?G²ÀÖ¾'Z?<¸Äâ¢Á?`ǂwÍ]?Qqp¬¹AGN4FGL J0240.8-3401¿í¤'I'LÀPcˆ†aÀ:øg³À<À–Î
>­@ó"¡ëx@œˆFŠþÌ?¿'t Õ'Ü¿¬lB|?îMâÔv?þ/r†r¿â0'9¿äC#k?;¿åsþwY¿âö?ç̂¿ÜtßzúG.¿Ü䜢7£AGNbcuNVSS J024047-340018?ïÂóp-B6?œâöɏDp?D°
†Ԛ?4aHȍ)&?{ðF>rÀ^?œà¡ÀÚ{6?ïÅ\¨CøË?}-±†ý¸?R¢fNÏ?YwÎUQ'â?xËCn—rÛ?xL)tb9?ïguaµ}?€Æ°èèy¸?cÒn÷(pÛ?YPW•«?—@ÉW?ù:Îcùð??œD'?i3–­óm?T_ͽZ
…?>Jb­»sr?‡R6o
T?h›yr!¥€?ï˜JKuÎ?ŒÐ‡Äpb?]'?M2ŽÏ?QkxŽ"]?†H…2Œøª?Œs ¯º!·?ïYIê¯W?–xKMÄ?aÌx'Ô¼M?q/tXŠº<?'3¹K?"õ¬šWq?îõ銷mY?ŠwÒýñæj?pU"í‡?gù\}ÿg-?-ieah,?ˆùèv¼îà?îÅú0ïG?ŠJ@<œm¨?p¯N°¾Ù'?c'QSµÙÉ?¤
¶ˆ#
Ø?‰ÍY"÷bAGN4FGL J0241.0-0505¿Ã3k–•ÇíÀKìØ]ú‡À:±²dkºcÀ<'£¤µW@µ×‡eåb@]OG"=?ÅAæ0 .?Á±Ï…ä°ï?ú\œÓà½E?ÿÈaMw×þ¿ï˜?ǖ,'?îóÕðaýK¿Ýá,Ö!à%¿â2ƒ
¿ä:"DÇ¿ânA§VAGNbllPKS 0238-052?î@]›Å!?Ç4º3pî?¤¥Jy("?ÇS†€ÉOP?t7^Ò¥-?auvOk»Î?ï©ZHØü?€±ÕÏ!µ5?]÷ãæµÿ?c%d)©~_?êŽi½Æc?z±Àö"&?ï…µeä?s•ùÕX1{?bî,ƒ?´Ò?a¢Îžv‰²?Š‡—ƒæ?pªíˆ»?îî˜ýšþ|?vÞYŸY?hNŒJÁ?`Wótah?šRÌ©ÜõÉ?sT©‰S‹Ð?ï[bäü™n?¦=òa®\?ƒüÇUÝ^Ã?¦†ËþÊ	Ÿ?…*mcÿ±?s
ø;á?ï7áÝl?˜&3D€,?qºO…šýQ?v‡Eß~Do?™ªoûq˜!?•yê/fÓ|?ï:!±Ö|N?€¸Ò˽£Ò?k#‰Œ"L?e·5BûOß?•Wh»Ž«?}d…z¥¦?íÁ2S©?­Th`\N?Ok'ã0«?w ^0Ã/€?¯Ü7CrÁ?ADÖº/"AGN4FGL J0241.3+6543¿Ø"Hsü@éh=;À93?Æ¿l'À;˯bXº¬@ 	G…z¨¾@°Ê1u?°‹lÛ Ú?£^î^(:˜?ót‰Y°u~@áj5¨ÙS?ìtxwàâ¿Î´
^'ӄ¿á`¢' *¿á'æ™ýl¨¿á׆߭¥¿â9LÝ~JßAGNbll3FGL J0241.3+6542TXS 0237+655?î¶Ud`|Â?'Û®¤ß'?d¯±Eù-?Tù±ÁµjÑ?£ZÂSpA?'6Òý8~?ì8ÝnÛî?²§(³Fv®?u£;9U!?zÜmð'Ù?¼çJUÓ_þ?±×ûrC'?îçÕɘi?‰hóž¹¢?pÜj§ø?dúÛ&^?žÎ,F¥˜æ?‡On•Cz|?í§ul¿?‡#/×tu½?'^!0?j¬^êZu?­'Å튇ƒ?…ïcÒ?ì¯C}5éO?©"Nû‡c?xÀq¹€}?jt;Ÿ<¤?¸ùݶÃ?¨ÑÖW'=¸?æ°Û—ÀÑl?ÆX=P:?ƒ¥QÐ+£?pm"eÔÄ?ÒÃ¥—åÌ?Âï2ªn i?í9hwsæ?ž¹1ˆæO?åæ$¿Ù?tÀ¬ˆ)Ê?´Gÿ⽔?œô‡Ìž›å?ê®Ó‡S?¡¤ÁßÁ˜¨?¥	•ó{±?…Ï£;ºÞf?ÂvßmÁØ? €¢ûÁÂAGN4FGL J0241.9-1603?ìh\IÏNTÀOýüÁrÀ:Õ¦Zr<À<'æ$Œ§C@ Æ*uIƒ,?ù²¶»éOº?ÑmÝÞÂî}?Ãñ¢õŽ?ú4°%Í#@(·'㟢¿ïþ"ÖúÎ?ïÿ×hE¿çånÿ½¿¦qì™­ç¿Öý€^_0è¿ê³Ù¡FŒ+AGNbcu1RXS J024151.6-160339?ïÐü­ÔÔ?"0Bb8?["³)ee?"‹×_$Î?q4ü7{ÈÊ?vK•kÀÐ?ïâ¢ñÿX³?o`=»v?8Â'O±?D½ÄÈ3T
?jDÈåj0(?kîÄð+??ïWÊ®SSÔ?ƒåRE@R¶?cÏÔ´
Õº?jýšß©?'Œ¯¢Û¼É?ûNŽÝÉ?ïiU³Tš{?pýŽäœe¿?Y°n€¼×û?C±'xÙÖ¯?':B¦U°/?pnÿã2¾f?ï¼ÇÜxˆ?y0K"³7‹?NS*Yږ‰?L_ÕPW)›?}ѬrF¾à?wÐäfuð'?ï› æÈ?"|'l+w?W¯XuÊuò?~"îy\?†H,ÂëGm?‹ÚɈÌL1?îÆuÍë?³EPçÛ
?l%+¥®Ô?q50tK0G?¡Ý%ë6?Ž£'ðmc?êÁ?‰v'˜ƒµ?d¤ÀÄ¡Ê?]ÞуT+¦?¢åÛ·Waê?ˆ›•F—¢AGN4FGL J0242.3+1102?†ï[Ð'¤ÀE¥ÄڐïÀ9¾½¨!óÀ<1Š¼‡@X:þُS@{ÇÜ£¦?ºýT)"
F?Ï+WÝ´>@Έ°=@$'w=N?¿Óh'cëý¿â¤ðñ5¿æ¾ð֗Pê¿êðþÊô¿ïù•¸c‰<?Ú6†¤ÊAGNfsrq3FGL J0242.3+1059OD 166?ïäë´³??`,üíü?]6,¬mF(?T²Êc*7²?Y©ü,$ºä?Pi9@D¾ù?ïÇ`ai§d?wRCq'`E?N@]vޏ?['ú©ñÍ?x‡Ã{eâ?s=&§¸®ñ?îþbç´bP?'æ:" =?Ž"*­¹ÈI?=Ø룃|?ñ»-×Ã?ˆ)"Ëš
?ïɉ+7fI?Zûò6a9?Päôä~|U?7¬-뛀?w-°\·?Vñ!]ÐB1?ï·?ò*̪?vDÙR‰ª?r	:_Ñª?iØnn9e?rVÌ¥•'W?jƒÛû<™ˆ?ïO²¢K'E?"þœ ß(?cü˜´ò±}?tE}þR"Ä?"Š¢W;"?'E¾c!a?î;)š¿Dµ?›g+)`?™¹äL"Ë?"Fñ3¼ùy?žàè띚?'MÂÈÀbV?ïRNG'm?{âWßù?jÒ
c°"x?X÷UpL©´?'[îÊ?Ø?xÄlÿ!PºAGN4FGL J0242.3+5216?É;XŸîPÀÚñˉ֮À9mmþ
\zÀ;²'쮤@3éހ~@_°&£Ø¸?¾ÁCכ1õ?˨]ס'@VùzªÁ@²¨ÑÅÛ?ïÿn	È֞¿ß"]ó%Q¿éßø…–W¿è,ñÀw)¿íA"d~.Ú¿ïóãðµAGNbcuTXS 0239+520?ïaGqiàÕ?‡Ê
|eF?tu…°v?pRœæóB?s`Àw8x?'ÓŠ•þ®?íØ3]ÙÂ?±ÅÌVÊ?fFA{÷ýe?rÕ¥³ã,Å?°Œ3ÙC?±N÷Éu‹e?î^áÕÓ?–5ùûÈ҆?ŒæÂ
^Ð0?†À9I*t?¢å3BoÂ?'²04eº?ï"B¬f¿–?qÀe‰÷?€â²1«÷¨?`ÃNæ™Yß?"FQUړd?j'OlP•'?î­DziŽË?šr0ƒ‡\Ì?.;½Fx/?}læ¡ë? à)n4ý=?–ÂCIo]?êrmœKá¼?ÃR*˜¯D?€Ðš™Ó·?Ža [‰ w?Å)AsN—?Âü¼/+ø½?í…t†?¡×£"?ºA£.?"¥
5®?¯šŸ5is?›Òu†©w¿?íVéæãú;?'d­'nm?A¿½ð÷?'''5º ?«ð±EØ?‰i'<À+¨AGN4FGL J0242.6+1735?ï蕉OۜÀBã4›èÿ2À:8.©`¶úÀ<-V@½XÛ@y÷šÖ°{?ÐÿR©úe?Ö‰bÙ?þåä`gHä@;ݹ"¬?ʲî)hÚ	¿Ö¸Éà‰B4¿á^'ျ¿åQ)=f¿íî6ߐð¿ß¡¸¡òƒ–AGNbcuNVSS J024248+173700?ï©2õ†æu?yÿ+IOïG?WÉð:ñ[¸?L¢éŽrN?'º–è7U?wÖî¢T:)?ﴕv§Ú®?y˜\–Ju?V!›&P¾?\*?¢Œò>?€^
"?uküô¤?ì6"Iâ]i?¦khJ?‰ñ?¦^ù'ó!?™ÖoVÝ®Þ?³`î¡@©? V—O2/b?ïIÑoɼw?mfƒ]"<1?j
=7{@?J~'åKä?""*b"`²?j´h1¬E?ïyb'ΌQ?"jy¬¥v-?bbg ò'*?W´<Îã‹?Ü1†Å2?'«èôœ.Õ?ïžÖ‰(?'ò"I§œ?g£6ãF?q3·hꫬ?™HEg]õ8?'‰r/?ëIT=ˆ»?©™æ-ŒyL?©E¹­Cë?›]ìÆò€+?¹8‰°Ù¬?¤Whih?îH°è£½?…Ì$V,¤§?x¿ŽŠt?cp'"'y|?¨]
®0­Ü?"uš®jAGN4FGL J0242.9+0045¿Ã¡cꂌ¯ÀI¨	ÃÎ ŠÀ;;éÿãzŽÀ<¤§:l™@±)Î/£?ÿÚ¹šû?ҏ¡·uM?ÃjÔL?ô˜çÂòXx?úiè‹Ï×?Í$Cy|n?Í0"W=(ª¿â~Ȃ=¥¿Ì­W|Ë	¿ïÿwy´!?ïõgÉÉãAGNbllFIRST J024302.9+004627?￧Á‹·??p¬ÙŒ(ºÛ?c)víWg?_[Oì°L£?v¦Š';˜²?hÿ·kHÆÁ?ïw|ÐNü+?ŽK7öaQÇ?mÄÝ!¯®?r"l(år?Š¯Æw`C>?‡O''‰?ï5´µÝO¯?ˆ³	ëã?w¾vASž?y‰5ëî©Ø?"YË­¥Û•?"ŸîL˜AÒ?î–}·Þ¨?†1Ê«Éí«?~†¾‡"Q?fÞaó+°"?¢ÇL±é¯w?ƒƒ¡!…±9?ïƒÒ'T­¬?ê˜96Å?z™v]Ó8'?x|_2p?¾ºîÜt¾?uÏ/)mŸ†?îǵӮ_Ç? B%ɦO?x²Œáx¡?}¬Ñù=3? nQ(|ûó?›µ¸à»ÿæ?îêÈÄ?"#[Q?~ÁãaO*?´Y°áh?ŸÚ.ðað?Ž!#SP»Ø?ìÚ
U¡ü?¡šÜӔ·ê?	Þ aZ?'N[ÐD?»Ö¸!Þ»Ñ?¡2ƒU¢ƒAGN4FGL J0243.2-0550¿ïÛ¯¥ÀKø§Å¬GÀ:Y¹'†¥¡À<aß 'á@|7ýÈBO@Æ<ÓG?½nÊc?"KtÈ~ßY?Ñ÷œ§@ @1|ª¤¿°àøûÔÍ¿éÔ¾³¯o¿êx/â縿é§ã¿³	¿ïÿúVrÓ\?ïÿânÁŒAGNfsrqPKS 0240-060?ïú_xû-L?VšÝ²ga´?2VŠÙî?Uv›®?:ûâÑÌ-?@YMݸõ?ïå`WFì?un²@~¨+?2Ej¹º·?B—®;çL?hVµCó?tdVOò£w?n'Ú¹?€h'ã¢?_ãr+o³*?ju€5s˜?"Wö³ñz?}hْ=éÊ?ï÷ìÐ+?6ê'?aTEC"?Ȩ•`ýl?NT!`Мl?4´@·Ž'?ïö¸Tßo+?N¹#ðŠ•?8ò.…"7?7gd&"è(?H¥lóü'?I"^:R?ï¯ÄlÅT?ŠË,¯/E?Kæ<ê ì?k¿¨ñ÷?'P{è㔟?†¿ÏÙߔW?ïLÎ1Ñ´=?‰·N¶FxŠ?cc®Ëææ?gü©šÕ?"ùÃìL›™?‰Bxý@'Ð?ïáßiä@?]ÔGžYܽ?9°«">Fg?0óí?jê€ÒyeA?[÷D 7èAGN4FGL J0243.4+7119?ï7üµC@$Ȓ‰ÚßµÀ9¡¬JvE×À;àf$ø
@Åo!JþV@-[h¢×?´˜Áò#?ª_z@ò'Ð(¡à@›ÅB궿ïýQœI?ïþI|JÔ:¿à­‹ßÙпßÖ³jû÷]¿æ"…€‡ú¶¿ämNí£ÜéAGNbll3FGL J0243.5+7119S5 0238+711?ïïôI
ƒ?WÇ)̹uè?=Ô[("DÐ?81¾ÕeµM?X¢VÇ®ö
?TOÞÁj8Æ?ï¿ò»/¨?ƒ¡€ºmÙ0?N´)· Í?XÎ	*?|02ÛÇ?'•ePëk¦?ïNwÀ½@?‡Àå¥ñ·?l©ÏXUŸ?mKÙ¥ÖÇU?'›Íþ#?†(Ó,0,?ï·àÕÿb?_
âó~/?Yy' #Ÿ?@uÈ6æÃP?~*ÏjÏ?[q°'.è?ïêB&ý+ ?^h"¾é_U?KúÍ'óßj?D}C$RÌ?]~KIÔY9?X4§˜C?ïy$%h?"ZB=R¡?`HKLg?s[ȼ"Œï?¹äã{W?'ýûgÃ?îäv†¼i ?'Û (?xù›–Ë"?{v÷r°©-?2éÁ'?ýx>¿©/?ïN™Ü	¬?y®C×¾–?p`\Áÿþ?]	pÁZ,?'5˜àƒ…?v!óÉPAGN4FGL J0243.7+0321?çø"y']ØÀHœ¡ô±îÀ;V¨°ÑåÀ<¬…\ '@H.ï><@šMô™?ÔçB.x¹O?Ófæ~y­–?üõO؅g³?ù¸0—!š¿ïÕv‰Ê½?ïÿEZ}$¿âîGÜ7£Û¿Ø8OfÆ¿ïÔF"
q¿î·N: AGNbcuPKS 0241+031?ïZ‹AÅ¥Å?®Kà_C
?nhÞ¾`?f†9ÃÚ°œ?á{ðLW?®IЙ
'¡?ïÛM Í´?ž«'¡uª?'™Z]ZUa?Œ‹{ô˜ä?–—é2Œƒ×?'¶Šµ ?íÄDüD›?Ÿ˜ÃÇ¡‡?—nÌS¥ù?'çö23?¨%ƒà.Z?—~6µË]Ê?íP2ûÞf?‹¾mÛÈ	¼?sõ¨àŸÃ?:xMûÕ´?¨qøb-Æ?"
²¦Q?îïeð¹€?"ƒHRæ'?'ó '±<¥?yLÁAåÔ?˜'Ãg‡«?'sØ¢'?íO"VWƒ?³UÖº^?—¿Ûym<4?¡3!õ‡Ò?¯-é:tM¸?­@þŒˆE?ìÿôw"_? Øb"?œFQ\¹Ë[?"|¹+]»m?°îËrï0±?šåé¼7L?êÉÿ½\cÑ?£9ÕÂGkW?©ÐÿÏh…?˜m	'LôE?¼Ç',Œó:?žæÔrÎø£AGN4FGL J0244.6-5819¿ÙàšC&ŠÀJ‹ …±…À9º'‰)ßÍÀ<0?\6a¼@ ‹'6û"¶?ûÜ ý¦‰?±
Þoú?¦å|."£?ø‡¿|'2@
€†µ‡Œ?ïaL'HD¿á§©Ý^•b¿Ö#ø'Äj¿ÖH:	ç
¿áÈ4ˆ¿ª'_ÁåÕAGNbll3FGL J0244.8-5818RBS 0351?ïôkeâó?TL»¹¹Ó?…t\ƒ]	?	Ó¶‡A ?U`Ý«6c
?Té=§?ïçtÃJS?jŒmEW"é?0ÐИôÈv?@õîß~¦?fqdM/ÔF?hv<^^g?ï¬ÁŠàm?yÉÅþöÄ?UX19qÝ[?dŤrç,b?'$—j÷?v¨îv—ÃJ?ïŸ:GF?a¿¦Å»Y?FTKdÊ?)Û0œ‡N?†Ð<Àˆm?`çìT#Þ?ïꢩÉΧ?`Ý3F7ú?06#þ'Ï?!Z<У¼?cV'¦Ââ<?`œdõÙþ'?uŒáû?Md	Þ[Ü??¾ý¡²?O·,Lüõ?9Œßé"?€FÃy`ó?ïyЭúF$?ƒç;­éÿ?WÞ²rlzÆ?Z?œ
ïW=?Žþ"JÑ·?'saK÷[¶?ïRY¥I?~¨½‡?8?YãOMv§?I^äŽßaÐ?œ—Ñ ?}ëÜõË[üAGN4FGL J0244.7+1316¿ë6ϟåäÀDÍ_™Ã‹À:h¢À‰ÈkÀ<+ò£ +@¢|f-@Œ°Úþ¾·?ÔR°+¬V?ÐVMênžC?þ¼g#û‡Ë@
Wxelì¿â^lg1g¿ã5V=ú6'¿åɓAÄ¿ç?¡k2Ë¿ïÿyݼ‰3¿ïûfKŽtAGNbcuGB6 J0244+1320?ïÙ=·h?e#¥øñ›?GêÛ=Ií?=H´£Ð?pz³ÕÑJ?cG"¿½þ§?yåIE?'HDq±ä?a¾¯¨¯£?yè;´%Qï?†£Ù⪜±?ŠÎNËø¸ú?ïEAçg>?ŒuŒ©YÈ?q´…"
B{?só­Æ©Œ?'ê¡¥ÕÝ°?‰$J÷R»?ïIþw%?p$9Qü"6?a+Õ¶HXŒ?DQwŠ»Ž?"¹{²+u?n'qU…Ö?úÖ¼?{à%5ì?VäßhßÖ(?Mñ­Š¤ªh?…¿eW³ö0?zXBt4Sp?îÐ<"sJ?¡s©öØÖ?rOriŒ,?€ûޞã…Î? ´=é'r÷?žQÔÛziÇ?	Û1P?•‡OÊU"«?|ȅìâ?|Ý#ó¬`?¡?S=Æ?"kGüð‹?î/ó.¥Ë?ùõÀZ$?nÝtF'É?_ð˜©c¡õ?«ü1sO?ŒŒ S—AGN4FGL J0245.1-0257?î¨Ú&§‰œÀJÏohیÀ:B˝!äÀ<oNÇ
p+@ޙÙ/†«?ÿ¨×úþ8?¿uÁ"I«ñ?¾8œ(À@ý"$½@
ý
ÒÁÙ¿¸ª½¬s?ï]&š¯™¿Ó86¨¿âѤÆôF¿á4C~"ë7¿à¯3ß«v¼AGNbllPMN J0245-0255?ïú‰‹&Æ?1§i "IÚ?!º™ð´º?y˜ÇÄLº?Ak,KÁl?-}v úý?ïéI^?jlЙ÷{?2•"•3ԟ?A¯Íða?dd:Csg?gpª.ᘢ?ïÅGèv÷X?f&ù×úY?R˲U[0è?W1§`!.?x©G귆?bd"¾¹DÍ?ïفÆ5¦L?O!=UVÜñ?G/ýÅz_x?.&~Ë²Å?pY#6›ß?LàÀÝëý9?ïõ¾ÌÀÎ?B¨O t,"?:Aêð¹ï?4\™éy÷?KãÖñry?9ybÂ¸:?ïÀóaKl?ß †j4I?BȘ—é+Š?S.*Ѓ?}-l#±Œ]?€x"ÚÓα?ïª!_²S`?q"$»>æ‹?WÕUÏð¹«?Vóþë˜?'|ýdÃƸ?pnèd.³?ï«­0¶gl?gùùá™ì²?V¶¤dbù?D=-Ç­s?'=ßJ²£?f¸?¿6òAGN4FGL J0245.4-5950¿ìÅçÁÖà³ÀI÷\¿ôw6À;#£Ï}5À<ÏÓ¦Û¡|@,¸aúœ?ýQ3~²†?Ò7'ßm
u?Ó¬ œîã@1õ`iÍ#@ñ_	zÓ¿éÆk>'aí?îþQ>¶ôô¿×3ŠÜgtƒ¿Ø§¢Æ¾ì¿ê¨^=¢ø¾¿ïò'šx¼ªAGNbcuPMN J0244-5948?臨0P&?ƒö†~¶ú?eBá ï?bÁãñA?€Áð%JÛ?€YxáÏþ"?`í_?‡×ܜä×Ï?b«È"
Ì?eh¦ö?ˆ&u›É°Ê?…Cvn¾›ÿ?ï!£ÇÖÿè?Š¶ÿaó±?|(X{ю|?|úF\?"Ápæ+Ÿi?"…þêÄ>?îíÕ10ŠÉ?x´3}úºm?ŽW¸£?bŠ¡…~‹?™¿×š%ó"?u<Uv¢U?ïL_ç2?ù1‹N?|pf4´\ÿ?sët)µív?ŽÀu'S¾ß?qâȳ?îâc5ôŒ?B‡JGÝö?s*[c¸?{mØ^f?žélÔ°?š¬ÁÕÒùÅ?KÄúp?'ß6†È?…-Åt¹œa?'®"\µ.i? Lyâ6nç?¬ VâH?í» ÚëôZ?'4	tC?‹=A…Ú•¥?w,[À
?­~¡îFó?Žfž^i0µAGN4FGL J0245.4+2408¿ïmeÃ07À?ÐaAcwŸÀ9«Ut¦›
À<ÁJ¸Šö@>ÎË)´"@._#|?µtîêXùÁ?´ý"€¢6?ø'"d¦rÆ@¸øU'¬æ?ãºO¼Öµ"¿äk^R›®G¿ë¹ÒߋkY¿á²¡bÃÝ¿è"£Y5ü¿ïöŠþøïAGNfsrq3FGL J0245.4+2410B2 0242+23?ïøþ$øKÅ?EôšxU"a?$­…Þæî?r$oè)?FÜ ®®?CY~éc­Y?ïã`ù{<È?mÑ(X¼@?5&ÊY~ñ(?C«a$—?iú-9Á»?k¶Ä{a?ï;z†ü*€?'Ï°_Œ`)?k"ïü7»?u§V=ÊÌ?•BZ‰?8™9ýp¼?ïíÀäÐéV?C²%E@"?6J›H¾è? Aû°"T?^ëoóý™?A¯]F4¹ª?ïß̀™ý?¢Uá"rm?Ir)1ähõ?zóSp&Åó?iÖôô¬5c?õ@}Vi…?ï²z9	¿z?ƒÉ֍ìÃ\?B_;^"è?NÃSa@'A?';}øüy?'ᛨ
å?îٗ¯ùFA?–‰•'Š¥?uœ] oy?xYË
0t?Ÿ‹âéóø?•^ê^<¨%?ïÉ …Ï•Þ?c0ir<
?TâùjRÄÊ?E+è à?uöþ¢Ól3?`q/ZE!ÆAGN4FGL J0245.5-4502?Üò6±,DÀN‡|í'hsÀ:Ð$qÏP5À<sóëõ‡@æ•â@÷ퟫ+'?ÄX½L&I¿°Ôí=ì°Ô?àíX]'@Z¹D.Ù¿ÂÁM½£7¿è>}i7Q¿êþdŸg¿ît¯45'²¿§".ÜÈ~›¿Ô CVìÌAGNfsrqPKS 0244-452?論úk–|?·#$‰
"?EWdI²
?o¦«tÈù?…JOi?¶Ëêí%ö?ï̇''Ç?pÊäYw;?PôßÙ£ƒ«?a'Ò±~ïÊ?u~ÿD—»?y%ûË; ?îíÙ鯠[?]‹Ù±?u>–×[Ø?z‡E¯c¼²?œõJ¡?Œ€p?´õ?ïî;pÞ(Y?HHÈZ'?"zb"9s?{¦q%fó?`œéՇ=?FËîñðn^?ïêRÍq?qåKèA‹?Eò®"¼?P…J9N?`k¦Ml?p´)tŽä\?ïeÍrAÄy?–ƒüŒHœS?]ž‰Mˆ'c?o>Lt€c?'li#žÚe?"AˆË>?ííÌvþå?š|Ie	?|!#Êã#3?'‰ eÛ?­ŸÓi2Ä?˜áB×Ê«?ïºqïHÌ?o"èJ÷1?D¹Àá5?CIg[w:R?€"ø'xx?mÖµ³}1AGN4FGL J0245.9-4650¿ßå–êŠÀNàC¢@À81Êx^¶oÀ;¿Œæ,ð#@­{MÔ@w¹Z)AB?¡™ÿÅój?½Vö†Úz4@%4z[ñ@0|o'4¿Ðnb×Vi¿ám=¾§p¿æL"üÅ¿ç}Ëb>Ž†¿éÖt€Û\³¿ìûgPAGNfsrq3FGL J0245.9-4651PKS 0244-470?ïΗ <A?rY™êrª?T\1Óèm
?S.}:-F?s#c':?nùB¯¦™?ïÚ=)Ååí?uz[$欮?D€8$»?_þçµß?pQd+b¬5?qþ(›î^?ﻉ0ÉT%?{AÓ#ô?c‡ž‰1[\?paØ8A	=?xw˜D/[ð?u'¾µ–?ïôÞù—}'??'}@9M™?.b 5+è?JF".?RuÉT£?;w¶ƒJ&?ït5«wVh?‹
ÑM/˯?aÍv÷j–?[p°%Óø[?Ž7rÑçe?‰AɆÿb?ï˜p ]ê?•'öi(b ?[dX;¢ºÍ?€…•žw?†wlçíŒ ?'±%ƒEï?ï'À£¸p8?‡mè¨Ð?k`¡¸zB?w²KG?"·®ž½i?ƒ'¬…î
Ç?ïâÑNšJw?^ùÚ͚•×?B²W¢Œùd?9\ûnKé?h'^\F?[Ô\Zî;ôAGN4FGL J0246.6-3348¿ëþ‰¼héÀP–=Ć­À;Òh;R¼À=ØL\Ïå@!«5MiÀ?ó÷ ›šœ?é£,àˆÁZ?֍˺Óûë?ë½Pù׳@¿¼§»›L?ìoè%ç}¿åú9¢8#³¿î†9[e?àçŒ Š9)¿Ö‹ 1¹6¿ãÒe}ˆAAGNbcuTXS 0244-340?ïi¯_dР?"îç_èKm?R†°[Ɔ?JAÌZ,°©?'©ª›îŠ?"›<Q­[?ïÃg""ų?ˆg²¿Ýÿ?Oø¯ÒTê?]ç…GÇ+?zM'ĠɆ?†Ò0 õ'?íûd#?ž¯@²¾&î?s-¡F¶Æš?yjäG³á?­â:c§dö?žRüP	ï?ï"vqÌK?sÚK¼­?*m¬A©?*¯ê¼3´?Šx¬×<|?sÑÙ0õú?ï+'îËi?™x§'ÕR?bfh®ƒû<?_Â2»¬?˜NR5Km?˜¶TŸÆW³?ïWnPë€?¤i¡ò=&?Wuîœ
èÐ?q²ûε?‰;f©xÔ?Œe±Ù®?íUr!ÒÚû?£êÚ_ú"ñ?n
ZòR?s0҃¹"&?´cþ…–'U?£ ð4ŒÍÏ?îÏvt?[Ï?—ñeñ<ÿ?1}wýnI½?B#©=~£8?¢åÎ
'Û?—åܳ⪌AGN4FGL J0248.0+2232¿ÇŽW_ý'À@r9¼º0À:ތ]pô_À<]ÏX˜GŠ@ }¼Î§îF@1jWX?ÈS¤|Ü?£ËF¡
bk?á(2F@̲-9I"¿äDÌMKn¿â՝ÖÀ¿äj‹Û¿à²Ál!'¿Éµû$#ë¿çÓû?PøÁAGNbcu1RXS J024800.1+223136?ï…íåæ¤?~ÉL8_'d?G<ô'çmE?6æ–Õ=Ô?Ì̎óÕ?}ì}éþŽ?ï–òUrx?…}§êx?Z0+ÓUŊ?a0J¦ç?‡4¾^Ó(?'.±9Q?ïMñ÷ûØ?€nÕK"Ÿ†?]«ÞÂç?Flº{®ýz?"gøy7Ÿ?€-í¬Fì?îõj«‹_?{-Bÿ1z?Rˬm‡?<à¥*Ÿ y? U´É?{ݔ®ÂÝ?îÖµëx£D?"¤©!‰Ù?Zÿ­½òx0?O}VN¥÷²?¡¼£ÞÑ?"<&5š?îä"ÌaS=? fæ»v¾A?cZ›ÿeÖh?o1«Œêà? |0B?Ÿ&Î4¡Š?îEÕOŸ?˜¬ë
³$Ž?fá2kXd?XÞêÍ‹?ª?ÿ†sÒ)?˜<cB Š/?ì¯ýfÑ"û?š¢o'EM£?hßÂÖ{b§?`ÏkÎàAW?¹¹³1?š›Ž®ßAGN4FGL J0248.6+5131¿êñ>ÏðÀçX}o—hÀ9NÎþÖ4UÀ;ÎDŽŽoš@N°A¦¾p?üçC:è3[?³YP¢"Ð?ÀÌê(þ&@©NBƒ2O@OZTŠEê¿á©åan/¿ãQzç&ë&¿ßÇRÅ؈¿ÖÔµÏZEÇ¿à=ÁA(iV¿éÊKéžtAGNbcu3FGL J0248.4+5130WN B0245.0+5118?î-hmgH?™ö2‰°'…?]»óÈ?wÅ£¼së`?¨è§§Vú?–ú'>Í2?é'òam?Á|¬·6@7?"SØkà‰?"f^ýJö?Ȳr´ä‰é?ÀZÈfc?îè—ÈLú?–V÷CÔý.?‹w
ô!‰ï?…ø²¿ìzÎ?§C³N´á?'ÃÉ
½'?ëÆq`aâ?"Žµ	î‰?[fôyæ«?mÐ?þ‡¬Ë?¿zòºr,B?'™'ö‡è?ꙩv}Ø?³€°¬•&?šJÀXû7Ò?•íÔAPÑ?ÂP{E5?°¡TÁ?âU¾$?Ë]©éÈÛü?'Äԇ‹?˜ù'Æ-ü\?Ú)…:ù€?Ê5‰OÓ?ë·ñžè—?¦CQq3_X?š•{	³~?ñ¢ ý†Á?»›ùåÎj?¢à$'†"ý?æ9ؐÓ?¦aÔé¾Ú?¡~ÔîÅ '?†¤ÖH'ŠS?Ñ\uW¬"?¥ù;ô*'XAGN4FGL J0250.2-8224¿ïû;>^NYÀ@Ӗ¿Ê…ËÀ9Ô	:;e1À<K›•ó@ŒGœÌ©ç@ÜÈÞ*Ã"?·'Ž zÚù?¯Åìûw?ó«TA ´@@ŸÇ™‡%#¿ÖÌ`it¿æõ®j}¿æIRŸ48A¿êA<ÀûˆL¿ëM'Ÿ'ç¿ïîxžwNìAGNbcu3FGL J0244.4-8224PMN J0251-8226?ïôBp?Uj ÛHåÉ?,8úyyÒñ?'û'ŬX?Tx\J$?S†dì:f³?ïä|Ä]?où	©êz(?4'™%'¾^?C¡C¥Oéû?hݱ"V©ö?mO#ɟO?ï,‡5F'g?"Ê-¶°`?d
qŒµ?tÄ`(öúŒ?—íË&çú?"&±½ì?ïò‡n@Fä??ÈçAhY?1f–²Ày[?+•ÿ*@1?V—}ß °Ó?=ܐ¦¯d?ïã	ŽvC?x¶ÐR½ý?>+¹õþx?F䗻¬°
?i0ú–+†?vC¥›ÙX'?ï¨vmçÜj?†M!S´H?FÃ0žß?UÓÇè_n?"v1†rì?…^RÖ¢?î"z¬ª©ž? ŸþÁõ)ù?jÒgo;©O?säÖ"EÙ?¦.½oÇ? ;<(:¶Ô?ïÙÀ¡˜?`Mogž?J\pÉ<Žt?9ÿʶń_?o¨aðú@[?]`Š¶%62AGN4FGL J0250.6+1712¿æ¾cݗl»ÀB‰‹`ñ²_À:àϹWÀ<*v­ÜF½@ ´¹‹Q'T?üB # –x?¼H%)Û?®Ÿ
át=ƒ?òÈ¥‹?cÃ@Ë:¦o¿ÓÏ"'|¿å¨HÞì	(¿Þ'1£X¿Ô¯$f‰¿á™Ÿ]þ¸Ø¿ÓyA쉁AGNbll3FGL J0250.6+1713RGB J0250+172?ïðÁs¨CV?M?AvGž2?)ËI^uÓÐ?Ær‰cO?[C¯Ê	`?JëupâSI?ïÔH+½Èù?q'Π)ˆ?=]4¹~÷?F™SŽ%?tìì×ù?p"Fe²ê?者=Ñi?x-m­±	?RðÀ…3`¡?SŸ,çåc?ƒ;"R~¿±?wl¯©B€?ï@ÏL;Ý?mLàJ?Q¸½£0?3z·¾Z?–ÊŠ¨:Z?lʨmçv?ïàS׏ë½?_ížKS"=??P•¹€í–?0U3¾­*?kÂÚIòn?]Z¨s±?ïzû²?Š¦U'ú0?PDäß8¢?_#""èÏ?td­ˆ÷¦?ˆxwäQɂ?ïZ"nËJþ?‡Íc@YEó?^&Þ!Dz?Sá¢ðûî2?'ÍE®Ì?†»‹…$"©?íø:§y^Ä?ŒÍÀx箌?g;Ýê?T¦Kµã?¯
ÑÇáÀ?ŒD'‹ulþAGN4FGL J0250.6+8435?ïŠßŽ_BŸ@6ir%·I®À:	L‰EŽ€À<~ÿÕ7ÕY@zR½'¾?ÿ¾Ø»gJ?½{ ¡yüŠ?¹íߨ,ì?ý<<& ûù@ð"W_´?Ë©©\/UÙ¿áe'¢xæ¿ã¨üþÿ޿כ#¿äÆ÷ µî¿ïÿ
!ANAGNbcu3FGL J0249.1+8438WN B0239.6+8423?ïæç( c*?SÊÇñ:$?FerÛ±R?6©ôÙ?c{ ·Ïr?P1Éä]g?ïÏ¥óLÆá?vÇs´êP?RêM;%?]kV`?srs!ü"R?q*=Š‰å?ï°Ù +g?k¨Üu†Ê?W"—˜ý?C¤úw2B?€åT¾ØGF?ià¿
•–Š?Š`ÁŒ?bÇàNޏ?vnÒs
iy?Q"0ZÝˆ?ƒ[t#¢^?]Ü…pô?ïѶ»à¹?bçø†\?UºA…â|¿?FÝ?g®Õp?qє2(¨Š?^öp¦"L?ïl¯ë¯?61Ýü?g<Õ̺S/?q‹¯ñ¾@?,HeýéX?‰9"~Û/ð?ïf¯Ï÷_?€Ãý«qõD?eÌܯFhÀ?h)Åý¡ë?pj€M	?|Q¶˜cQÊ?îÌêŽv^?ëÇ:vv?‹^ é&ò?np3V]œ?˜³]¹9_,?yÔDRyÑQAGN4FGL J0250.7+5630?ém<«å"ÀíÊ"Îa"À9ÙÓr²À;çÙÉ4'Ø@ ˜ù(öCi@Büý@´?¾2ÿܙžw?¡]¡à~Ê$?á/¯4_?ôlÃk$;¿çë«_>ÔÒ¿Ûï—<M¿ã'#? )¿Ö2£uæa¿â{ÒÿkÛp¿ä	•ª÷ïAGNbcu3FGL J0250.6+5630RX J0250.7+5629?ìXTpMM™?­Fø½0?rb\Ã.Ñ??dÕ®î!?¼6µ@5?¬åÈ¥®wc?ä»°­‡b4?Ó=%
·¥?øÑa€ÔI?†œTž$ß?Õøؘ=µ?Ã8k˜÷ª"?ì¼^s‰?ŸÁßÔ~?…‹žYFî&?yŽ¯ûñ«'?·j'C^Ïn?«›ðN¿?ê',ÏÁɹ?šjÄÐÃÁ?ŸïññÈ¥c?~É\Š"{?ÃeNƒ›«m?˜Š4M™Î¹?é×Âõ©m?²?÷-ö~?ƒ¸ÿne?vö¦¼ú7?Çes]€õÅ?²Á\Õc·?ղ҈¬#?ÇŒ±døŽ?…b9¨d¯ú?'Ü9±u?äÑ
Õc/?Ç—ßÛq?é–éÈ?ª¨Ö?'hE×Åä?ƒYãö²íß?ÉVµ'S£?©_ÛpŸ<€?ãmVÂ`ž?ªtäà=7±?±å²w7"?˜+';Ž^n?Ô«ç:pû?ª'mœÕRMIXED4FGL J0251.5-5958¿î½ÆaΧÀI¥£3vOÀ:ËGxd•¬À<»É{´Ú@øTD«@ÁÅàIS?Ç)%=QD@?ÃzO|jÝ?ùͼì"øù@

yæ ¿çOÊB®Ñ9¿åm÷T_Ó¥¿Þz&ÂaŽæ¿á°.fDØw¿æŽ"¬Ï¿ïÿ¤?åÉAGNfsrq3FGL J0251.5-5959PKS 0250-602?ï÷†ƒ??êé¶ òs?, %?0?!_Fç}f?L—x{`ǂ?:ªûï‰.?ïÛFÅÐ?q¶<x
{?;5{¹Èä—?LmÞ:÷??p©žÁl'?mº,g	J?﵈¾]¦Ø?sŠd´ÀՈ?[ôËhN–?jm×Þ©R?~>mâ{F³?k¦¦çš·\?ïї~7¾?V;r‡7?Aÿ܏>™?%Uãûèë?tô<¸ "?UQM‰M'?ïî4Û¡H\?QUÛÇA´?A.‡]3?5¾ôȪ	?ZÿÄi2À?Lÿöˆ&«?ïÜúÚZ?ˆt$ŸY''?Iø°ªÚ‹?TV"ªÓ
?Š)t°‡ö?‡…ë?ï‡
ӟ`?y›K÷U†¢?aq°>E8Û?c–€2àêö?‰á».ãÅ?w+HC˜i?ïwýò«ûé?wmOè	d?UÓ
1ځ5?EaZŸ³<?F!¼,/x?v±(eàìAGN4FGL J0252.8-2219¿ç‰ ­ŠfÀO£n.²À7ÐUÑì"À;¾t{'H@²«Yà@òþ½x?"Ð-'Å?¶փ¯Íc@ãrý›¢@XxPô4¿ÅÖSeª)¿áãА俿å¯>Õ'å¿æ—cÉÓô¿èâ­[µ³¿êªàHª"½AGNfsrq3FGL J0252.8-2218PKS 0250-225?ï͎A·?‰'c'^í
?WîJ",?hßߞ•'³?ss'Õ)(?ƒDÜ<O;O?ïÏçú$ɹ?~¦ö^I—
?JxF€|Jß?[¦âD:¼ô?t¼úfÏ?zV:Q9x?ïÇñÈÒ
Ì?tt?Ÿg?Yۆ[Æu?câyï?u:¢("?qðŒhXVø?ïùm²‹?41ˆãÎ^•?%*'ŒÕ=?M
\x?Fœ~èiáÀ?1PB
{L&?ï—<êZì?"|]™oDŠ?XPå5ôž?RPÝW§c^?‡4Ô,™d`?ƒÈ~Î+
Š?µ3Ä?ð Ûe•?_Û¦¨–
?yó°¥çW?…aýø?ŠHÊ~{Ìx?ï¥qüǑO?'ׂ$¶We?cþ»¹j%?q³tÐ!A?£Ñܤ+Ô?~ß.˜&¤p?ïð
`ùax?Pâ2w'ö?8bHæZšk?3ຍµ]–?YÒ¬%í?Lç`M	'AGN4FGL J0252.9+3834¿ïÝê)L;À2ipÅdùÀ:[>¢Òþ?À<YNÛʗ@Ïa&
««@%Ä'â?Æ"?ÃYí\9fÔ?öȍ$@Q@àÃA]ÃU¿á¤1£:á¿ä´|ÿ…ä¿èE¢>Ù°¿è3ªÇÜ£¿æuI"ˆÁ¿ïñ$€	AGNfsrq3FGL J0252.3+3830B2 0249+38?ïր|q?f
£Ö?IÀ¾É€V?AûçûGÑ?q‡°7¾¦Ð?csã—¦?ïÃÊýa6ž?~Ú¼[€Ù?QíÌ¥Wæ?X&$&8A?yŸ*ìŽó?{}âŒÝ2?ï\Ÿ&»‹?ƒVÇ~+™?k''ñÙý?qÜx¥¦í¾?ûÖ@7)l?v.­ùá?ï™2"?Gò?dÈȍxP*?b"?"1?CL!@5«#?…,}ðk?b{%§âV?ï–z\ßÌP?ƒOµ¬îÌ?\®&ɽ?]ÙÁ€£g?†Ë¨]ÍR¾?€øVÅOi?ï<®Ïa?–•.ê'õ)?lÀ/
ìH.?y11ó{«?"ä$_äIÊ?"wø}æW?¨Ì¬/?•4°ôš•D?ð}=è?€šßÍÚ
Ç?£–EÌôØ?'ŽÑd ¹?î՟	×*…?'³†b"§?yLNpO5?c/^§R,Y?žù*fÂ?€x,²ö—ãAGN4FGL J0253.2-5441¿æ'
Ê ¨ ÀKR.±Ä2ÊÀ9®æb IÀ<†Õ™úèi@È܏ú‰@åZ'"Ã?°uuøՔG?°óéœ;_}?ø=Žkh-ç@¯³ÏzÒ¿ÛN0¥lÕ¿árç]ò¤x¿ç»e4Ù¿éIiÀãàe¿æÇ>îRX'¿à÷ÍaGBµAGNfsrq3FGL J0253.1-5438PKS 0252-549?ïû¥vWÜF?1.¦Ï#Y'?;uÎm?4H넽?>…Œ¿gÉ?08ßÎ Œ?ïîí«®^?e΃߇µM?+<$Þåe–?:©^ãõ}Ÿ?`2P1‹0R?cÊ4ü¿äF?ャ=,¨¢?cá2‰cò;?Tžõn¼?EïÑ*Ó?|%9º$ÃH?aþ›¾?ïü¹W~? ž²Pî?eÓ;è±>ýOCš?5'3±bý?1ÆB
cÌ?ï÷7U½Þ?D4èO-¬Ó?oò8ñZÍ?
nŸ¹]Ô!?P0'!ˆS?C8.¿O^ò?ïÈðiŠU?€÷¡²C?>±nzUŠ?S0>"»í'?yœ´Wë6`?+Þ	õôý?ï‰t©'ß¡?yH·xyf?` 4"ì4X?WcXÓÍeX?‰zȉvTÔ?vå†Ñ½Å?ïö1vx5?BÒÊç¥ÀÔ?+µ˜—\¤?·M N?O5‹Öà£?@ñ*výÏöAGN4FGL J0253.2-0124?æµ´Z@ÀI‹Z ÝÆÀ:s­<
ÍHÀ<xåÕ²Nœ@׫¤^º@X¿ÜúAz?¾1Ò55?ž•AÆü?â^˜?ü4'g"#?焝=èîÁ¿ÀÆïh-:÷¿â·#\=¿à"Ñ~7hw¿ä	ˆ>þB'¿Ñ6¯ÿâxÜAGNbll3FGL J0253.0-0125FBQS J0253-0124?ïÎô¦å?i±du¥:Ž?F»½îQâ?7çN)—÷®?u®5(ÊQ?g Ë«°5?ï©SsΚ?{Í/¹¥)z?Ye"/wVl?Xøö¿™j?'~r{çdÐ?wg®ËgŠ?ïƒáˆ½ö"?sÇ> )Ê?b«:çî¢q?ZóFbªº?Š\φ²À?p×ÒÎê?l?ï±hJõ¥?rŽç|º…?xÃa¹®?Wn'ïPÚ?™ú®Ï4?p[¾:m…?ï˜Y÷~bm?xCÚI[ïb?[ö…a…?KúÖ¸èŠ?†j±m®€È?vÕFƒ?ïË¿S		?"/5NuÂ?h†[Ȭmc?pÙkg"P?˜õ¼¢`§0?'-€pò".?ï2e×¹ÿ"?€zÍ5†TW?jØWp…sO?añåFÀ}?–X:O‰
?}t9ðµ?팈ÕÎm?‹Âþ.þ÷ë?Œh^{Dö¨?rš«äáÖ?°³qèíÃ?‰¯ë€ò!ÔAGN4FGL J0253.5+3216?ï°yTª§3À7ÝÝãu…¾À:LŽ¶È¥À<VU°5½Q@°uÔ@9D$>û?»
Äv)?¢äž5ñ»?ç\V­‹¾æ@N;Qkƒ¿ïý‰-:Ë®?ïÿËA²Q÷¿åü&¡ÕRW¿âå`w9¿Ý-` Ô¡W¿äƒ«ñŠòAGNfsrq3FGL J0253.5+3216MG3 J025334+3217?ïüöLfϲ?.®2\ÍÌ?AuŒ³s(?ûrèÈÎ?4el‹ŒJ	?+D¹ö€?ïðAŸ:K?b[ӊ1ð?$7gƒ¥Ké?3ɏMpsß?\õÔò¤ço?`Þ£?ï´#ÍÜä"?xÚ•?V'àkw^½?aÝc/7'?€&°€×O	?v`Š[‰L?ï÷žŠD<?1i›½¦•?)âÖDÉ9?ßߋý ¤?N`›]û"G?1:\lý?ïûE_ts‰?4½óªx,Ž?–NÈʈÂ?¦þÑ,?>/p½û¡=?2Jeò/Š?ïÎÞ®\Û^?{kÅ."ÿ??M«^øS=?Nüìz·Vf?v›Î4NcØ?y¿kÅû"?ï‡Éö-Ä3?€E
Q¹ÅW?_e½k?faU!Èç5?Š á•JÜ?~¦7&OÒ?ïëÏ¿Ez³?N oöœ;:?-ö¦ò¥†? š.AjY>?bPÖš5l?MX^¤¤AGN4FGL J0253.9+5103¿í‹KßÁ5À¨—š¼À96Fñ'À;̯,¨Õ@Ä7B·`@‰Y_í¦a?±Q
¸Á?¯†ë8üv?úôš ¨4@×ÒÙ+Tí?înŽ¾tDu¿à7–oB­ú¿è"ÆÜ	¿âù'žªz'¿éI^]®[ó¿ïÖýÓ*	AGNfsrq3FGL J0253.8+5104TXS 0250+508?ïÎ	³2?hà˜ö¢Y?DY™$~1?3¦'ÄDëP?vmH%\í?fî	Ìr5?îì£åq?¥G JRm?C}×lì;?TãG¶k˜? é]ó˜l?¤üîî(ÊÌ?ïOÁÈ  ??¦ÕµˆF?hà@,Ò?dÎc?'ëÇÅÄe?×Ø*6Qü?ïÃøSýòÎ?ZÒK'(â?TPO'XA?7ó>Râ2?xïÂÒíà?XŸ~ª9ØÉ?ïîEԆ¼?§ÖèÄúñM?SÅw´?DY×"c"â?¤柛a?§Ú?Ù¸,R?ìOÈ޼ʇ?½¨Ù†!J[?V½Û"Ÿ"?mË@4íUU?½&Á HàD?½«'
KU?î¿O5È8é?dã‡ãß?wnÿ°°|¬?s½
y©¦å?¡,¯¸R?Œ‹Ç@hG_?ïPIêZ¥?|8iÜ@}?q+#˜)7Í?]=ÝSSI^?'«ùÈ¢Sy?x13?!ÇßAGN4FGL J0255.8+0534?ëTìqíÀFÉ2µ^ñþÀ:½âïÙÀ<K4-@&ž'a™£@Ø8 þ?α^œÃo¬?¼µ‰9O,
?ñ£ø,Ìç¥@ªdSç‰?ҍyYˆ¿çCÞ¡¶sš¿áå­é¿¿à°
fóT¿èžP¸7ï¿è­ŸÀ¥!7AGNbll3FGL J0255.8+0532PMN J0255+0533?ïÉþ±ÿʄ?|c'áÛÒ?F{UÍÿ?Põ
ïòÀ?x1D ç¿?x¥w^v·?ï»G}±ËX?x™l?P,"Z0?T¦ÿ§KN?~Q>e.@¥?tÑyd??]²Òj?vÏ2ÇÚ ?ViݎÅæä?GƒžJ›Œ^?ˆlß
îÅ?uâÁö˜ïÄ?ï/Ñh?Z?q¼ù,>?^օB'¢p??¥¨1õ¼?˜w9*?°?qr_K•Û?ˆËbŒ?{KŽšB÷?S6o$uä?GÑ=Ꝡ?‡4Ïëe>H?yÊV:ø6!?ïTLÑJ?Ž"Z,x,?[4Í2"z?bËNâ*õ?"Ë餩*!?‹Xì±¢?ï)¢¼¿Ë?‡Ø%"ËÈ?dæŠ,¹ê?fŠ|Žk?˜.׃z~?†pP·›¬?í»»BÖG?'JG·‰?pŒH,Oxh?]
b¥o?±bê•f'?\êît2AGN4FGL J0256.3+0334¿ëÚ¾¿EªÀG}BÙÏÀ9÷íPÐÒìÀ<AåçP@Äþ¹®â×@"2A›«Ã?¶Œµ°{ˆ?'YÿáÞ=?ÝG!&Á4é@	$¼¥BÉ?ïû†ô{g¿â¤'ýuE¿ãÖÂ^ß´[¿ß3Žµâ¥¿Õú}¹©"¿ìÒ¯/-5AGNbll3FGL J0256.3+0335PKS B0253+033?ïÝÂ5o"£?eÙ]þ?7čäÅN©?0—msŽ«Ÿ?oE8óT^œ?dÆKÃÀ¼ ?ïÝPÜ¢"ú?l¥Ë݊Ék?75Ã8‡¹X?Aü2Ÿ+?oÈjÌÙ`O?jƒ)¦#¹?ïšÐ_m<³?yJjïy€c?T¢¶O'?U!0»R]?†È¨¨Ý5?x¢<†.0?ïª>Ñ];?`߃Ï&%?I5kÖGf¥?.Ó7¯k?ƒÜôø*?`r·;¢?ï½5>3J?vDVô¾æS?MÂlE"Z?B~0+¸D?}­2J$C?tëB£ÿ|4?ï¢ÐÓ¨ÅB?‡½µ{Ï
­?@ýTçi?O²s¥{?†;õÖY´?†÷q_?Ší?ï/pN$XØ?‹È'MV2?`Æ}ª´Ú?`''1¤÷?—ù&ˆZ ?Šì3rݽí?ïtš;?}>㫎¡2?a	ÂO´ö?MfB0|vª?›05°n¥Ù?|}¾±¨òdAGN4FGL J0257.0+3358?ïè.ž	ôÀ6K<>t°À;ëÔÏÑÀ< ˆÛ¢@ Qg¢P¢Z?þÊTg`aj?ËY
Þ*m<?ÄGøý'LK?øz_\†é"?úW|5°'?ï'سiy¿îký^åé~?¾Ð_("ƒˆ¿àEéÞö!ÅL¥Ë¿çžÑ'ÙAGNbcuGB6 J0257+3357?ïÙ!nåé?fŒb-Ë´?:GwË"Q×?0ª!g¬?qÊÑ#Žoƒ?ewî؟À?ïvùzĆ?ˆ¿-Ö;±=?m
¾¨F"?pÑm¸@«ó?ŠþéÛ1‡?ƒ")R?ïH»‹ù?ƒ'°c}…i?bGêÎã!?XâbçP
¹?"§%£q—o?'ÿèjPŠ?íÏ]ixв?ˆ1ä썹?HDf[.?dú`•?®¸K*"·?†Ìº×w»?ï—ñªÁxõ?'­‡2´"?OÆ24Z_?E*í™ώ?ˆX紝?'"š?îš.ü ¿?¡*"þ)Z$?:&ºztñ?Š‡,ߥû#?¢uÙû"ds?œ/·&lò?`S8?'™\βâ?h𮋭•?iF0ïÂ_?¢¨ÏÉÖá?þ›²ë¨š?ê$ÃÌn®?¡6Ã@Ê!?'…¦­XË?=*‰¿§?Å<>²öÀo?¡4ãuŠæAGN4FGL J0257.9-1215¿ã_N5(gÀLmîËûµÀ:6¯-•À<tÞë³Aá@ß?@1É@oœp
¯?¹Þ!
j¢?"h|ü*?ÕåFÁ/Š²@Õw®bS‡¿Úƍ«p¿å¯¿üò¿è…xDµ;·¿åP½Š'¿êšÏ>—"¿ïÿ€^	J¬AGNfsrq3FGL J0257.8-1216PMN J0257-1211?ï÷Ðh…?Apv(?0"ï'ÿ'B?#P@ôÒ?Hte™¹O'?<A5}°òá?ïíVºKì?fU+zµo?-ÝR}û8ñ?<rØñ&ñd?aÔϒb?cëä^s±³?ï¾@¥a£ß?o~lõP>|?X#ϬéÞ?csÉɳ?zÖ¹f9Ú?h||9?ïôÐÄJ"›?7šL¦DS?*K¢Ò×?ôc2Cîò?SQ¬
¯?5zº3`?ïî¤?VMát£Â??Ç,iÆûá?2S78ô?ZÆ-LNJj?S±Ž¶Ç;æ?ïÃn•<›D?¸}"˜3??͇'Mɶ?Q»Aôb?|KÜàà¼Ù?€"Ü(
?›´±?y£$zº-?\#0Dûa?Qâw Û?ˆ§3%À[?x(½¯ê'?ïâ]¹Ï)?Výµ|¥Í?C®úë@'ÿ?5 óÒ<X—?h¶‡£'Vâ?SÙT
"f¨AGN4FGL J0258.1+2030¿Ö¾»^‡ÂÀ@ªé>›AÀ:k$-ܲÀ< p­E£@x¾'²!?ÿa­ê‰v6?Äðª7 ¨—?Ïuéüˆ|;@WÚè'®@	úâ"tt¿ïþsÙ°k?ïîQs	?À#^~æe¿á­:*ž9<¿æ¾J''?¿äûF'+½ôAGNbll3FGL J0258.0+2030MG3 J025805+2029?ïì YÒ.a?VÂZü¥€v?B.²fé¸?7R3ü1?]¨Dœ?SÈòCr$D?￧Xý{?zÕ°–vQ©?Q"Ñ¿'_?XÁŠ¾#V?|÷ûõä?vÑÈóðñN?ïN>]Íi?‰È°;$Kí?pÅøª–*?ukœÀDp?'îАxI?‡¢â±
»?î¢y½Y†?}ÛƏ=+?s^…°O[ç?XÁ¥Øoê?£l"zfeŸ?{±®I(?ïÖy <?nxß|Š9´?Y³ßkÀ'?W\ÊìWîˆ?m½_«'?fÏËÚ±?ï1iõs_?œ՛¶&?gUñé,Ïû?€µEͺ˜?–è!£$?–©µ×£ü…?îmî†
©??œ9þú'–?…þtҟP'?…þ‰s¶Ïî?£¡znÉí?—Êþ³¨"C?ìþD85é?—¦ØÒ§?'´£Zj‰&?s·ƒ:6?µ·IÑníÕ?–†ûf¦ÐAGN4FGL J0259.3+5453¿é'J™x®àÀ¡!MW¢À:Œç='[À;́I@»²@ ¹zæ{¯@È>{?«¡ƒóÀ¿¦z¡÷Ùb?ç¥F`Œ‡¸?ñê2]ö*i?îpÿ¡á;Å¿ãçOš¿ç}îãx	ý¿ë‰ÝÏSÊ?кý Ë¿ßÎ59©AGNbcuGB6 J0259+5451?å7žãìŠ?Êr»fükÿ?µñ8³mÌ?˕¬–nõ?Îƅ*KØñ?Â3ÔIT?à½?ýñÞ?ÉÉÁŒt9…?‹ž
'Íþ?"-¢ê?S?Ý­B,êU?Éß*XªL?éJ¾E±¡3?ª€ôùdûð?'ƒ‰»>Õµ?‡*M¨Ì´Æ?Ȅ•±,³<?ª)l*¸ ?åçêÚvP?±Lw¥C•?ô³R»{?sª¢ÈBם?Ó°W}·³-?±IàÚ«?áb\7}3¡?ÇOÏ5²¿Z?°‡Ù­Ï¿B?¿L:ì2M?ÙQ%È¢­?Æþ}&¤ã?͝ä¢ñ ?Å*'Þ
ù?‡×÷{¶ªƒ?š"L­™?è9[i:ß®?Åû''Òy?ãp»Ê¤‡?³T±öl4?œWØî0?'MoÇ?×Y
ëö*?³¼æE†×?Ô}"¡©?·ŸéX¸l²?"gÛ>Q4Ö?"ØXvW®?å%÷™æ+Õ?¸©dºÃžMIXED4FGL J0259.4+0308¿è*â-uó¼ÀGbŒ?>qÀ;zVÞ3'À<¸ÁDŽP@"uE?¥1}?÷è»ûÄ1?×›Á''?Áº	戶?ê&¿AžÛÎ@Œú–Àn¿ïÿ`Ï‰@?ïÚ ri¿ãÛJ¾ëԿَK½m´9¿×QmZ÷Gu¿Å^eYAGNbcu1RXS J025923.7+030736?ï×È!}^?lmô£Î?2q»IR)í?,…8âyâÍ?rôÓr̄â?jºüÅÒÑ?ï½= ±É?SM¥'Z½?JQÕ_æŽC?StŽþ
ù?~þ®£b?|œOPÃ8?îû¶l­[?'ð¹Äð?Uã?nÆ?TŒS+¿U?Ÿ*þ"¹/?'ì6Ø*å6?ï$Y,'a?€[y€¥þì?GdëV/ÿ?86[BÕ?š¹³ ›"j?€J•ntye?ï Üv‹w?¶ÄôÐoÄ?Dؓ!1?:	3Ž'»?†‡ñ׊Ò?~á³Qç)v?ïdÊ{J	u?Rʳ?V"Œž;ÆQ?eä1'HN?'‡Éïj	?J/(U—^?î5؞£?–Âž	?]"#Iå^?`Bîõ¾
?§±gûî¢?––DYß
?íˆçÈP¼0?›«Ù—sj)?SÊw&¹èn?QIQÀ'Š¶?³i—á°?›àâ_YwƒAGN4FGL J0259.4+0746?ë®é³žŽ²ÀE¨×¾˜V£À8¦ºò¯µeÀ;—ïrBÓ@qieŸA#@ùü£T-?¥½'&?¯Äà^ô"@	ž>^à`(@:ÍûXü?ëÄS­úпÞϸ$B`¿ã1¾Ý`™¿âgM"—¿åÈ×tÆ{z¿æª ¥gAGNfsrq3FGL J0259.5+0746PKS 0256+075?ïîyÝM?X	ýáíó?!¤¬.N[?•¾£"•¼?`䶣"?W¨»¤G#Ö?ïèÀÝ}Á?hÃqÃâyz?2Ëì0Ë?C&%£\Å?dæeÚ
\)?fVSK:?ï Âšï¯ü?'q­96?]H×>P¬Æ?hì'»ò¾0?"&>KË˒?€§¨£"C•?ïéØgÏ`ë?Frk¿Éw?+ ¿	˜l?Zø)gn?dmŒÈÖ{?E4£
|]?ïÚ©¿V—'?e¡ºûîR?+}[L…'?xўlM[?qÏ5€•¹?e0ÅgQ?︮½m3_?"Og…A?GeàÏ!Ø?fIaÙõæ]?€]ò'ñÂ?'"p0h?ï>ÔHŽ‡?†ù^ÿ~u³?a2ÿäØ®l?h"¼¬Hg?‹ãŠîðË?…ÉZÜ­[?ïÑ "
O?`r'Möq?=‰c
"©œ?.òžÂr0Â?uWa

úY?_EË*Ô£AGN4FGL J0259.5+1924¿ïžÊü4¶ÀAÒܱF_À:y–°±
TÀ<#/V/@óôëû@õ
3¿?Âwÿk±?r§Î2s?°nD_÷7?ü€íÑ)Rà?ïl¤nò¿ã[QàG}î¿æ››œ©"¿âk
=²é¿ê4:WÎô¿Ýe5#xU&AGNfsrqTXS 0256+192?îó¦Çï1?"ñ…Ø‹`¶?q.´º";?e³ã¤WF?;ýý´ZÂ?'o.NpF?ïOiËm?ŽË"ŠÞbC?oI¯Sn¬Ñ?mJV_6·?'3Üâͧ?ŠÃ£±µ*?îý xA@?‰½—©/?xn7@ãé?wº'ö'?š2¾Ã¥¾?†»ãV¸.Á?íº3ÀKßý?…œx7f?'Ú†ØAÙ?`ì¢~?¯¦"{z/?"&±T'Gã?ípõ›£	/?§™œ;èìò?†C4ã*"ü?zžm0âxi?±¯ì†ðWh?¦ãÙ8–?î'ˆ—Ø?¨º@Am'?~Û?H@¾¾?…Âê@"'–?ªTþ,r"?¦d`¸¶?íîrA™†?›YÔ55'¾?‡ÉmJDí|?ƒEpÈ£?«&€Šá–?—º}ûê'Ñ?édžlɵt?Ÿ7×°÷d?™§Cì·ûd?N'òªÃ?ŬýÏy$"?žbF?V7AGN4FGL J0259.5-1705?﬌…m¬ÀMcðí=…À;,>׬#àÀ<ªçcQ0@ Ò{ÿ)ì8?ùâwXüñX?Óô¸#G'Ë?ÙAŒ&êO•@¼[ed?þoKº">?ïôGe_M¿î½8À:î?Æk¼f£".¿Óx‹A'¡¿Þx'}sHL¿ïçB.x¹OAGNbcuNVSS J025933-170540?ï¨ãpþ÷?{¤:Œäā?GŸµ,¿?;"ª·ø³¤?"M(c¶²©?zïH6jÂ?Æ1'??‹A#k'÷?j½v|nö?s'?x\þI?†¬ÎH°š}?"!L÷l˜?o{§°?"™¼ßÈ?wAøT?}%‹ô£'"?¢F z€?'¾r{yqQ?íC\Ïþt?£]Š;M?{§úÝb»q?bãcÛù?´-Ul8Ðf?Ž¦p¾]s?ïMvmš5?ŽsÀ¹Ú6?Y™=ª¹8?R¥"#*?"·žoõ¹ß?§Ötö‰û?îÍwþÉ?¢Î´'>A´?y΍ý‹Ø?†bþìžh$?ŸÝ\Ö´pú?Ÿ¼ønf:?햶Zš€I?£K|Ð#4?yX±ûè?~*Cu͘ï?±´Ì1
Âu?¢¾
Mè"?éum
փì?§êx¢[½Ÿ?†¨®€¬?{Ù\(¨d?È¿Àí	?§ªSøûAGN4FGL J0301.0-1652?óºÀM-«KrÅÀ; g4À<€îßFL@xƒ/ö@A›@bƟ?Í@›üu[ø?§ê­ÞJ"¹?à÷¦ë@šÐ"Øi¹?—ŠØ>M¡?ï"=ý'·¿çU4_ƒV¿ÝRìÁ´À¼¿ç+=e¼{¿ïúª@/ðÞAGNbll3FGL J0301.4-1652PMN J0301-1652?ïðz4Š²\?Qø0¢çûl?)X«ÈÕnm?*ó"ð`x?[àŸ!ÏÑ?PŒ:ET'´?ï왐ºL?f»Rãe?+.=@Úf?9Žöˆï0Õ?a³‹Ë4M8?cÑÞsW)v?鈴n'Fÿ?rFÂÆ´eë?Vôn/À-s?Ns0èÁ¯?ƒu'Fžµ?qoÔ¹×,ò?ïÕô|‹Ž?S©ÏØl?FÍ¢¹?-éò•wrM?r§l·gª?R%G+E{?ï߂'I¡½?cLt_fÛ?:âÑõ?W?2 mˆ†÷š?m!tö§à?b	§z)%6?ïÅuRg€î?½™¼ö´?E‡¯³ƒž?fÚ/Ðîë"?z"`ÍÓH?~y/Lÿ3?ïcK3wž?Xs	¾?`U~"2
?[çO@˜>*?'‹ï"gR?èýéË?ïžTÛ¾F?mé"ÒJ?VH:ºe?E1£ésÇ?…©å?€
·?l§ÉÜM5wAGN4FGL J0301.2+2546?æè}0ÇÀ<ŽDR?gõÀ:ö} >ÏIÀ<dX£/D'@ÿÜ0B@ïêÄ.˜š?ÇnšgtÙF?§±U¢ô·"?àÊzw•bÓ?þ5&U)R4¿ç™ëcÉ?ê>zúr!†¿ß)ùc-Ì¿èiU./¾4¿âG)T ¿«-£SN(AGNbcuGB6 J0301+2546?ï §Þ^x9?x%û^Pz?BqŒø0Ò?1¾`š°Bˆ?†®ïŽ'?w'ÔË>B^?b…c?~'F];Ø?XõcAO¢?]@ͯ†¤ú?"÷ƒÓ¶UO?zÞ̒‹ý?ï[º¥Ð+?€Ý"«‰¯¹?dà.šše?[ð?"$Ş?'ì¥y.'¤?´³¢ðŠ‹?îÉ8EP?y¬=jÒ?sYvm}í?Yî¤ß|Û?¡P.ÿT?yÁŽ Ú:%?ïBUA8Ú?‰ýʘ*ˆß?R©E›¯
R?CÖDªA´?–ŠÇ¿}Ì?‰lm%B:Õ?îÜèíÙ{¡?™à)hÀ?ml¤Hí*K?w|¼H? Z¦áM?—"6JEó?î°$5>{?'ÙXϹŒ	?r"Ax?lª$PÌ1+?¢¾›48Ê?'¹¯<,ÑÑ?ì±ÈW¥¶ç?–1žáì"t?"É(Ã碛?w4°§£U¯?·Ø˜*UTu?–gk­©ðAGN4FGL J0301.4-3124¿ïë¬íšˆéÀN¸G¡A)À:ÉŠ ÒÀ<¼¨¨*V@áÚûä'@/S6L?Ã]:ƒ3¦¡?±ÒIäO Q?ì¼^'í0@QºÝ·¿Ò=?%¯½¿Ñ@{EE¯b¿èe¥@–É¿ÓüνgÔû¿éWÌÊæn¿éõF2ê8AGNbcuPKS 0259-316?ïfÊÙqd¶? ¦¨%ž?ha‹H˜	?x¶®pGé?sdIØF?šç4ŸGm"?ïʺÑw¬_?vüQ£Ïf$?Mˆõ€?S\'B¹?vñ•x\'?sª)K3HB?ï8G«Kƒó?ˆq¾ú Ff?p'íuÛÄ¢?s>¶3Ú(O?"ÖO?s×j?†¬diºmu?ïÊf|G
?c7?f#³a• ?JÈ1™Ÿ:ƒ?†Dy®L?aÖ³›°)?ïUzW"ëV?TžåIJ–?j†HæB#š?gll8®¹?'ÿìÕ¿¾?‹Kõío"?ïl>£Ø??YùP{}?\ºÛæ̤r?e»-Wñíd?¬Ž«äPË?Ž	Yäۈé?î¥,¾`3®?'í{üÏ!?y™¤õýÖ?yÙE3oC?¢yÿ|JÉë?'Œ	Ý%>ç?îÙæfYƒÝ?ƒ"kXÌF€?}Bœ*@6ü?j|0vA/2?rŒ/:å‹?€¡•Õ'ƒäAGN4FGL J0301.6-7155?á÷IF+C·ÀDã[ÕìlÀ:"ïÙAOVÀ<Š³Ï¥Å!@'ñÒjÆr@óÕ4z[?¸a=݆.?°¸9þå‰î?ô+¸e6»~@Ÿ®†¨?Ðt=$à¿ã4ÿ@'lT¿åf‰l$ìI¿èrNf•`O¿ì°a¬m\¿ïðȊGìÿAGNfsrq3FGL J0301.8-7157PKS 0301-721?ïð&©À‹Ô?NeÝMý$¶?82íߣ£Ö?/Õ.iI÷?Y¥ð¢dx`?J†#¼|î?ïÞÏ{¨Â×?qY9\	²?;Uû—¿ÇW?IVú"?mÅĹc©•?n–ÐÇoI?ïÄꜰ>;?rž÷<È?UþzgüÈÑ?[C‰p¶'?x,@Y?qQLíO>y?ïæk(´ˆ?FýŽÉù@?PÀÚÙIà?2&U+Ý?aˆ‹žëþ??CÁ@óŸ_?ïÙ§	v™?cZÔ¨´wÀ?KZ¢[?>v"E?o'v‰²?aš
¾Ü‰?<pQT?‡ÙqfmÊ?L¯ùRŽG?`Yò±®#l?†O±O5Ü?…T¸œœ¶ã?蘿o=>i?x¸5ºAÈ?^ÝG/rÁ	?`Ö2Á9@÷?ƒ;W ¥ ?tÁßJ@,?ï¹-T¿Å?hPÎg¼[?fSéõD?Á?Rœ"Ì«._?x?`č!Š?dm‹3ÓTAGN4FGL J0301.9-2731?¿%'ƒŽÀNŠó¡LìBÀ:©·¢åsÀ<°XaÀå8@-^g¿Ví@ˆÐâ2?Å.ä —?»œ©'ý?ö8›P˜Ÿ@3êrúôR?ï¬W¿ãž"Ô]ºÆ¿ãÓÂT£ÆC¿áÝŸ¤u–¿ê2ËŸ¿ïÿ3Qf$!AGNbcu3FGL J0301.8-2721NVSS J030158-272754?ïÜ3וJ!?h¿1MM»?E]"÷´øv?<jÑ"°Ò?ntÃOŽFI?f‰×	Ä2?ïÞGà"U?o±Ýž#?=ÍX»È=?E»ïZÏ4à?n9¾"‹óš?l(1æ¼?ï¯m´lu?t"j/q¦A?[™9ås±?f×t¢ž&?€±k¼ùZs?mŸè‡8Œ?ïÁê&‹Y?UðӒ'?YshG\?:0"ž®ËÛ?x®¼Œ?S¨­ÊZW?ï ®¶·6¸?y0P™L?YրIÐOW?NÕönþÂM?"™'Kô?wl'FôÒ?ï"ŲڻÖ?‰'0ž!v?RF\¿g?`ˆý¼®¸?ˆÅÇ·ôm?‡R lä³2?ïo50ÐÇ?€XÞ»	r?e³e'¹
Û?i7ن©³?ŽÅåÙ·a™?|Èåk?ï`ü	%m£?s©ËKc?lÎÉâE?U¯R4ªÓ?F¥°ó
K?qÉß´ç‹AGN4FGL J0303.2+3149¿åç[=ŠÇfÀ76˧2ßPÀ:hµ}$îÍÀ<@¾(Å@tÙrÍ|ö@i=Š¥
?Å-h±Å4?Än³&ˆì?ÿ»iGÂ6q?ÿÿ—ðw ô?爆ìî«D¿âÁ²‡§(οã%Ɉt®(¿æj}ík¨Æ¿êHuà+ú/¿ïÿùëñAGNbcu3FGL J0303.0+3150B2 0259+31?î‰`ªsÃ?–»uåÉî­??œ­&?rªA4cA?£.5²O?"D½"ô¥?îáÙ(G>O?˜èKF4?ƒ—J÷*‡~?'E‰8+Í/?™ù5u'«]?"xóHZ¹?îÞËeø
?Y³öH8?'Ù5/ö‰}?¡O*þ?šÐúÝ?†K
zI‰?ìS7Of^?ŠVH__ùõ?õãÊÔÊÔ?uQ3ى9H?µæQÌZ?†haüýË?ì(þÁ¼xl?«—'6á¢ú?!KXì?'§ËC\a…?·oÈÞØGg?§~3ÏùÇ?ìüö›ÛÆÃ?®Úü=è>?šÈ™/"ë?žëÐæ:pº?±f$ÖôÏè?¥Í"»ìÞC?í\ª•¦? B•™b?™+ª|
ª?ó)b6òT?­©ðX¥?–þRH$Ƅ?æëOe˜á?¡j3Dböé?±2¥†YB^?Ä'ú?¸?˺£þ*Ž?Ÿ7_`åRhAGN4FGL J0303.3-7913?í…U§ÞÀAý´þyîÀ:F‹yEf<À<c@þÍÐÙ@rË7@‡¤¤—?½ù
†? Ç†>?ã	Õ×7‰Ú@
€«Œ
e¿Ñÿø^¿ä"\0ýN¿égþìډ¿Ù@ÛýÂ8¿ë¾Ïÿ1N¿ïÿLkAGNfsrq3FGL J0302.5-7915PMN J0303-7914?ïðäC-s£?P\­^Ӗ?<^÷ÎÑE?5
®{û?W»°½q?KT¼òn"Þ?ïáqv²0a?pD£6"w?8/#Ç%™­?D
ä+%ÿ?kˆ¤à¼Ç0?m.W†m¥œ?ïéÿ\0?pãÂ%_¦%?\(ψè9?iNš£Ìü²?wjw>d7?f&NÓ2¦ ?ïßH="v?J²Îl×áJ?KÏ`»"@P?0Ì¿ëùâ?iÃê%zD^?Fµ{6'?ï㿈ý¦E?aH-°j~?MU»‹KA?B'5øQ?dë †Ån?\æ讉ÿ?é@Jô?‰´OØya?Iqԇ81°?b\…L:­.?‡Âèfi)?†ð]º_%Ä?e¾†õ?y{¼ óŽ¯?`öy{#˜?i›èt
Mh?"J7—Ø?u½{'ü£?ï«r•Qi?j<Z´DS?d¾L'èíð?QÛú$Ä?çGá¤?e…}kÝ<AGN4FGL J0303.3+0555¿â¤æ¼ž=ÀF-û¹À;Tšù*4À<‹ºˆ&ª@"¡ûï»?øÿø¨ó©°?ÖwºKÀÉ?µÎî:/Ѫ?âºcslß&@bü]^*?ìÈK~ºE¿ïÿòß0&¹?ïþ'¨'Y¿ä«­Bm㳿¾Ã!¨FZ­?‰R Ð‰^¨AGNbllGB6 J0303+0554?ï9¦oÉo(?— 4:¸À?4Þ*cÀ4×?)Æ]	^Âó?˜w¹Y"T?—'ƒwM§C?ï–tYªQ‰?N»ŒÎÿ?_Dûø?oeß
²<H?†¨°!–4?Šµ§}n&
?íÔ>6_Q?¡oùPþ?X´)Gãøš?]´´'í?°û?9Yp'?¡‡tª¬#z?í¾uß*G|?'ƦÒn¹?B
£öS~¹?89kÄ« ß?±è;ÀAñ^?'½ÛµvX?î=Gè2?)?¨8œ{6²8?E#ƒê!?=ºÂ.N&ó?«Öõ\È^Ò?¨);ùÛl°?îõ>G
±?£i®ç¬?iŽ2Ò~U?}F‰Ž(?ž&vÃÒ ?¡Ò) =jÍ?íã%²IÇ?¦"'ö±P.?Z8âQõ½E?`Æ£Cø?·0H¡éÑ?¦š2pÀ‡o?é"E"¡Ì³?±eœôLUŠ?HGìßõ^ƒ?MÃÃ
,J£?ÉÖ¡Ä­»Ý?±gùÏQpèAGN4FGL J0303.4-2407?áOòÉ-'xÀNŠ›ÏÔ¿À7¤¿Ä¦ŽÀ;'­¯Ñƒ@g½ml
?ý"«þöë"?•p³W–ûì? w›ºR™@<ï>çœ\@š'ျ¿¿u š"¿×ö‹ÂÁ[*¿ß
X^©¿Üª½"µ·‡¿à·4µs¿Ýìðƒ¶-yAGNBLL3FGL J0303.4-2407PKS 0301-243?ïô\iž`?GrÖ¦èù?֕Ýn&'?ÄC=Ó$?V)Ê9B'?Fïᇫ?ïîBY}?f54â'8 ?1²Pxm‡?LY-BM~?^ NTLä"?bIÑé—âÎ?ïFTdӋ¥?'Éo  ò>?soÃSq­?'=ÙL0‰?'Y'Žva?öq¼ä¾?ïð2ÐÈì?I}a+¹¼?	ìûÂò >ù4ðâ{?_.Û`¿'"?I0^ªR©Ä?ï৙˜9?f,é²)Á?"<Á"2@u?nî.}0k?n5%Í®
?eÕãrY§?ïӔQ±"¢?{t·Íå8B?@äòöÐ8œ?SîGaå?t8Õndí?x€½.‰?ï>¼7:?"$/òý\8?qQ=@"?|Åõ'·Æ?—ðêð¤ä?"*ë¥
1?ïç<Z›¤?[Xë@D…?ký«"Qæ?LÃ+&ìˆ?hdc¼›ÜÕ?[(~ÑM¯EAGN4FGL J0303.4-5232¿ã3#¸ØqÀKVx|é_«À:NÇw"vMÀ<mÏt@3ÏDvQ–@Ð"<jêZ?ÄE¡Iç*?ËЗ;ÊÜ@c±€@,@@rwÅç«¿â\^¿âⴕžbV¿ëf¿§ C¿é©Ì·ÔD¿ïþÒ8F˜k¿ïð®SeâAGNbcuAT20G J030328-523433?ïöøÊ#°?CZ ¨ъ?A ;	¬
æ?7ŽRÞýê?Bü› ¯E	?7O¯‰ºIë?ï×´šüÆ?{vž´ô^?Hæ×"è?^äF/Ì
Ú?qÈֆ©?uow,g«?ï›ØçÉc?{©êP샮?m°Pì?qÚF<ºBt?¦J(V"?u5e·œ¾W?ïì­Áªì?C'3«QOw?Gˆ³1O?/¬,:òª??\›rC2¿??	ïÍQlj?ïì*ë»ûC?^Í×:?Råþæ??R¬ÿØ?TÄ)Ž¼jX?Pz8p€æÛ?ï†Cyã'?Ž‡ëP®^Ç?X/Ò]1íº?j(¦I Ì?‹i'@Hµõ?Š"¤±&ˆh?ïOð])µ?‡sökŒµ?wº?Ôó·?zvÌ$…?J?dpHæ™?'	9æÞÍR?ïÇ2ƒ2¥?e	ÔÂ[?`ÑéDdLs?P/†E²€ô?sþ
þ§ãy?`x|õVzAGN4FGL J0303.6+4716?ìk-†SŸÀ#µx_.QÀ8rÆ	d,ÐÀ;˜äXڌ©@ˆƒÇ =@Ǧ†è½?¢§û\,PÁ?´Qç¾Àš@H<¯³·@Ԓ¾Þø?ޛà»íŸ¿ÜŸF¡úç¿âŸA¤:¿ã=OK—®¿æЎÞT´¿àíñ_©2êAGNbll3FGL J0303.6+47164C +47.08?ïRáûþ?+xW>P)?UÒþµÀ%P?R	^Õ¡?"b3냵ñ?ŽÐö?FmÌ?îñmóoñ!?¢ãz·vçM?[ª Èüúb?oò÷²=OM? ËÁ-3?¢13œÃ"]?ï'Á÷ÄP?'›™'žŸ|?fÝÇ<WI?r‰Nðr«?…ØL¶%¼3?|ºÄ{hõ?ïmgƒê'H?jðOÛn1?q^&Ëù—¡?PvæÏF?‹÷"Ê=?gGðø¯¸m?í½ÓI,ˆŽ?°¢hNÑ9?føÍFB?géù¾}jÃ?±YŸNQ.?°&L20G?íŸ'3åN"?¶?.ÂtÔõ?tï/Àetõ?‹ªÔ^Ï^Ç?±·Ód˜:\?µ)åB³3?ïb?éáë?eϖyÁ?k¢Þ³rg_?wˆAÕÿÑ?C¦çÚµ?‡ðƒüv¨?î½Pn"—³?…'Œ7O?'"Ú‰:´?i²B¯À^?Ÿ
¯½ˆ¼F?'J†áÛý—AGN4FGL J0303.6-6211¿é—«OÏvÀHYå\ËOÀ9Q³ø^KÀ<êg¹M@¨3vë@Ùb<5:?®É)¥?¸S´²ú"¯@c¤%
×@‰ˆ)"´¿ÞpGÛá½ ¿à6¹?|AÅ¿æªiËuµ¿äZTª|?ì¿ë(ÔɎտïþ²í'¶AGNfsrq3FGL J0303.7-6211PKS 0302-623?ïé)¤5¡D?Wÿw4ýä?9ß8{K¡ƒ?,+­K#¶?cštٛe??VHÀ¢jÎ(?ïàÍÒ¨¦I?{&څ¶?>³	(ðŽ(?VÊo⻟?k[ÌaÉoß?v‡Ù¶Ï7?ï©QÇ·©?z3"Í?`´is÷÷…?_ýù+Ï	?'6;Ý?vƒg^Ïh?ïê]©©\/?EÜ[ÈbY?5(íZ2€;?Ñ*²¦c?bý8p!	Â?CäÕX=.?ïνùÜ`¥?nCÄ_ÉÉÍ?E'>xýã(?8ïÚÙL%?uüL•7"?l°ê<£
8?ï³Ö ³~È?†Krú[kÛ?DûÆÅLú?Y!·ÍÆ£¼?º»wlÍy?….$Dq¸Ä?ïp·—Ó¾%?'è3A3Cª?kB/cY?fdé,_Ÿš?™Cn¥á?U8Þò?ïÊÐ÷\v?bŸ®!äå?L%/,^`U?<,5ƒÈf[?wÞ_·l´?`hŽ½l®AGN4FGL J0304.4-2833¿ët¨úýžÀNU<æÀ"À:øÕ!/$±À<˜5¤&»V@! pe˜¶?óV¡—"Ü›?ÙÃp,¸Å¯?ß(Ì|ðÁt@j¸A$@eK#É3?ï÷D9ë´?ï¢.(1wq¿å°'b"s?Ë´¯¼пݳÿ¡`bk¿çûûŽ7£AGNbll3FGL J0304.3-2836RBS 0385?ïÎZvC(I?p¡JöBñÓ?QBäØ–?QBÆ0I?t'¿Æ
õ?nZ³s+Ú?ï°ð•Ô¾?'ôNï—?] ~'¾Ž?f‰"ܨ!q?€ʺ¿ª3?}v‰kóqé?îôg¿ñ‹ã?<"§)Þ?w¶!À>R?yOãˆG,$?›…‰·Ÿ?ŒsåZ+Rf?íÐ72 ¢?'µ=‰ÚQ?zn§¯²7?m™½sÅ÷Õ?¯¹a÷F?'•ä.Nƒ?ï¶ZWíÛC?u³6ñe?a	›ÑI5?X+‹+:>?|ND®6?sn¤æwð?ï4Å!1Óã?›'¾b†?oFÀ¨*Ü?×jÂi8?•~ƒÇ'úÎ?•ò‰âÑͼ?î¤'"?›\W$ò+@?~ÿ"·˜P?€h…}•q?ª_#>-2?˜ß'uƒ§Ï?낕mÝJ–?©KúÞ¨O?ƒÈÕ¾XUÛ?ƒú"$™;?À¹ìŸÐë?¨°Ay7}AGN4FGL J0304.5+3349?À¦—®ÝÎ}À5\ÂÅâÍÀÀ:ˆÝÇÆӏÀ<ڀ¶–@ò1Xèy|@æΆ
pœ?Õ
å=‡?؞œã¦3@_¶™" ä@%#ûݱ¿ìºÁ5¿Õ?ëAµ!_v2¿ê»à¡¿éáìžú+«¿è²2·ã0¼¿ïéXü˜AGNbcu4C +33.06?ïÛD;ï~?v³Íñf¿e?f¹·Â´¥ü?n¯7Ú©6?\'Ñ?cЌsæ¨?ïI¹r…Œ$?—6ü™Ø©†?|Îͼ¹"Ä?‡t£HÛ@?*< –?ov§Éˆ?îƒ$Á;°A?•ÞYŽ§þ*?º…®rr"?‰Ëáûžå? _~ªr?'Céæmo¶?îÖV…À?†Õü
!øë?¸,šÞ?s]‰—ÁÛ?M/Dýl?"Àš–Bé?ïÌm²Ç#Q?~.Ûâi?sTÌNÁ:?zmM$º?YÔ[«²(ç?[Ê]Q)ìJ?íä¨;?i?±ÿÊég²?™¤d‹¶P5?¥Ú¾ÖS¯?¤ìÃ3Ý,_?¥¶Þ¹^Zÿ?íÇö9éÁá?žIr…Q?•[À)­!?'K˜ C"?¨¸î€s$\?–¥´º§ô?ë…®ˆÈ?¥ó
pÜó?«
$º'6X?–'ã9nãB?¹²Áwà?¥µ)SFµ,AGN4FGL J0304.5+6821¿î!-ræË@!.Ÿê$ÌÀ8Í~¼ž`À;SàGÓÔ@^^ߎš@[\|ؘ³?°­xH¼?ËK­h¿@U§L	ÃÎ@H®ÅzÉ¿Åçû;õún¿â½:ZMS¿èXžâ¿éÄÜޒÇî¿ëyóa2¹¿ïþú¡Ç:'AGNbcu3FGL J0304.9+6817TXS 0259+681?îĒQYl‹?dA…÷Ê?—7 GvA?••Áÿ±~ý?6•Å!þE?…ás'@¨
?èfm+ôÇà?É"v@V»?ºIʛ¼€ò?»«­zÅï?ÁAfN ?À
ë¿Åìù?ëã…6ê?ª2ØHÅ°h?²ÌŸêå"?£Ý¡"¨`,?¬/_×z'?žnåV•A?é>|I°?¡îüjø†?²›Â,6Ÿ?'"•zQà?ÂU$ùÎQv?¶Øº{)?ì¼bõvAÙ?±qdÌ¿S?ª÷lXyÛè?¨wàߙÒ%?©BdRµ»€?¡»
0õ/0?㕈V·?ÏlÞ~ê°|?È)´«D?ƕÁŽ¼W?ɗžAÉùß?ÄÜÛ|ÊŠ?éS"GX??²(S˜CÞE?¿•ñ<ª?¬£.Er+ë?µÎÎÀÔ[?¢ØøqnÁÏ?ÝKœaûŒ?­ êKè?ËÙñÒ¯~¢?«4ƒ™–Ù:?ÔÇkFE#?°.…ðt®AGN4FGL J0304.5-0054¿ïßAº=0ÁÀHXǟfb5À:â,[ØÀ<žBuÆ@Ì0ÐWpÕ@X϶¤l?Â.ú(ûvÙ?€åƒõ9õ¼?ÀqU­±~"@³>†MŒ¿ïû–ÿ‹eú?ït¦Àž–.¿à(é}Ý{q¿å
*Ž:Á¿Ü"±þ?`"¿Ê¦2™°?ÎAGNbllRX J0304.5-0054?ïÐhCœs$?q@q
ϐ?@ع7¯‹?7)§Ù
ÁY?u°ÛN°ò?pkC""?ï܆õõ ?n"¤ý£Ù?8%ރ1¼?@ätö×?p:a*]eÓ?l[­tõ¤Í?ï;ì¼ù'?ˆ xiŸá?ba¯KHZ?c´æºQOŸ?–PL}ïàq?‡¨¹°?ï³-äÙ*?`æE$!¥?EÅààiÄ?/` Äb?Øa6ðç½?`¨ŸsÌù?ï¦0ç\"É?r
Œ?O¡­ƒrûÒ?AóÂî"u?"y«FNÑ?~í	Èö'?ï'JŠ_6i?ˆҔÂ,P?I"¹Ç‹äU?aCï9"|R?Š!Úw-ª?†˜kçW‡?î§XÖÓ-[?'°¤Ù&?mÙ½MŒPŠ?oà«Heü?£¬Ö»¢¨Ã?'ëæäH3?ï/öŽxd|?~|§téV?YÂU>d®o?M‡Åçt-'?˜e×廣?~)G7|7AGN4FGL J0304.9-0606¿ï¯K½BÁÀIû5ü;OaÀ:´BˆCÀ<|vOèu @Þä^9@æCåÍ?ÊÅ4'$E?¬nÊcª?à52F¤)@@â)é•ö¿âÄâˆô'¿ÝG­¾"¥¿¿â$ýh %¿äL<ÿÂ«¿ã_iG¿ïÿþó…õAGNbll1FGL J0305.0-0601PMN J0304-0608?ïÍïæ=V?¤Ò…3:ý?B<»Q½?qÅÅl¿Dœ?vÀŒ-eŠê?¢šV^Ú¡?ïÔ¹PN³?qÇY&×,?>¥Fˆýˆ?LI½Œò4¬?s¹Wåf?oÁ	xŽVü?ïtpp3!s?"u`—«ì?\'òçi?b"ZàÛ©?Q…¼i"?ƒ'òe‹?ïÃÞ~Ðëj?W"
`I?<a¤Æpó
? €oÊ?|J¦7#è?VÛá@åáæ?ï¨3£Ý?"™OX"®?Gzâ|ü'g?@dl¥EUD?"h"ßß_]?ƒÝô{¶.y?ïq.2¿?'‰Y®½°4?OFBQzép?]ýÒ­OA¦?à
D¼?üá"Ã2j?ï"×y4[?Œdlˆ‹ÌŸ?el )×?]6LÚ"?›¿á	£J{?‹rÚQÀs?ï^f˜€Ñ?v"³Æ.ä?M偘³Ð?; ¤ŒC?"DøÝÓ¯?v'ù®)6AGN4FGL J0305.1-1608?èoŒ·«IèÀL•!Ý Y§À:€'_ét£À<k7…¨K@!	‰Í?û€N¤¨ÁU?ªÄw=Ï?®. |wJ?îÚ³	­'ì@
þ"™Or?ïÆÛl6Š¿çµÞÿT^|¿×ÐPåË¡T¿à"H÷À–¿».ù<ÂS!¿à.ŽˆÄ_AGNbll3FGL J0305.2-1607PKS 0302-16?ïìî4sn?X:úò`ðZ?!6æö^‹?pQÁhLm?aþ]dxÜ?WÐ0"øn1?ïâ¿{¼ ?mC8#³êx?4õè??Ž˜Ž¬?j¼å¯ô"?jêbñÿº?ïyqQb.…?€—l¤D¿?L´úÅeÿ?7Ò*2Iã?Ø[õiç	?€'ZIk?ï±»Œ¼)?b½ô®só?/H
îŽ?.ÙÐ<»;?ƒü¬!}G?b±g¬¨?ïÜY:êó»?i¹^?Ú@=?4
êä5?'9EwóÜ?p''
>7	?i@\c?ﯯéù>¬?ƒs'vøu?@‹éŒ÷Ã?L×CÑùR¶?ƒFÞp–?'¼Á»Æp	?îÙ§—ÛÎ?"	ØÁ®¨Î?S8Çu‹¤?Z†'è¢yf?¡ËÀSí|?"üÐf-ˆ.?ï}9Uzö?€û†E—Jr?C§"ª¶?8:lËå,?œ³2ÌÂ!?€ísU)áAGN4FGL J0307.4+4915?ïúZ"ÀGc€X€À9
¾.¤XÀ;ªQ­q½²@µ$h?ÿ	GŒ†‹ ?­Nçï'õ?¸ Š6Nœ@©ÊAR@ãTpšœÏ¿ánoês¦Á¿ÝÃT~–¿Ù3$º¼)¿âÎg öo³¿ß6#¨{µ¿åû¦Ôë?AGNbll3FGL J0307.3+4916GB6 J0307+4915?íÀ
%­d?£ÉI"Üa?kã–ÃF€^?d–Õžrfc?± Êà?n¡?¢NüÞՑV?ì—ÚNŒøC?·	"
z?qeŒ¦àâ«?~Þó›ÂS?º*ÔÄ+Ø:?¶|çŠ9ëŽ?íِ΀n?šÑ'9×}?‡/¯ŸóÙ?"U¨¬»¥?¬›1¯†ˆ?—Ž™÷''!?íWÝ3ø*?ŠÉÝrüÊ?‡Å~÷BFk?e4/=úqT?²HfÄYÄ?ˆ°Àº‹O×?êÛtØš#?µÅ:ø?~҃0#ÆÈ?tEx1KpÒ?ۘ†bôÜ?´;Ý}ìa_?祂?#Æ?ȎªP(¿ð?Š³7ùG}?"&
8©Ü?ϾÅOLe×?dzõ_)?뀤eO?¨|>{!¼?"çZ"™?Œrhij›?¾ÁMª‹b?¦g}­f?êNÅN9…?¡Óß+õ?—ÜtKƒ?€ƒä0ÆI?ÃÌ(|©|? ¬>¼6ÂAGN4FGL J0307.8-0419¿Ç6€
¸{îÀI%ŽÉ[ÿÀ;`ØÞ¨—À<°yixiž@ÆðŒÅuÀ@ڒ_ét£?Î'
)¤"?xÔ â«^Ó?¨D<ߞ$ˆ@åGÂâ=?ì©ðÿ±üg?îâBµ‡5ê¿Ý‹@»\¿Õp^aàÜ¿é'Àoz¿´ŸEÀ~ŠÊAGNbcuLEDA 095522?ïÓ9–'@•?g½V'2?H¥ãÚPˆ?;Íæ{w'?sNxM4Œ]?e®ªí°?ïÒ#ôÚeš?rÒ¬˜?Cs¨¤ñ?Pƒl|š M?tŠ—R'yF?p+JϤQ?ïa×1Äb	?ƒo>€´{?f@ƒÒTŃ?q"ËšaÜd?ý	Fó:?Ä}…Ø?É?ï«R·ƒ#?dzŠ"–Ís?VãM"Ò"
?>ìî;ª0=?'Nèq:²?cOöžë…¥?ï£EU…Ô§?}7¦â»Í$?\+/¹[?Wt~mt?ƒ©H‡±üC?y¬©V|Ç?ïŒXì
Í?‰gŒô²?QZAj¨&?jj¯tý?Š¾·YtŸ?‡™W,?îüi²!?ŒŸ.KEb?kíÚ
¨	I?qÿ/4Eä?œð7œ4º®?‰(^¡ai?ï!÷dX¢·?5g¼¹ñ‰?gÀu,Z?WT¢XTáÌ?˜Ém›?ҋó|±AGN4FGL J0308.1-2852¿Ðú	Ä­w%ÀMðX>…vÍÀ;`Á¥À<ĦÚ'Q@À$¢ö@_ƒôç?É秄ô¤?´ßª_‡?èC ´@ZÖ¼å¤?ïãq¿_üÀ¿ã0
¿0W¿Øò@#Ü~¿æH¿AHõ'¿Ö
HÞI"¿ïÿ·Û¤%AGNbcu3FGL J0308.4-28522MASS J03081686-2851054?ï´¹ñ†s*?zNeÏ¤t?A6€ê…Ö?4‰£iE?¾šÂcê?y'ûöÊþ?ïÕ0¹ë|?tã|ÚЪU?BA×
O+m?KR긪?sÀΈù?rŠ+¡FFÃ?ï\	ü?'&=ågp ?_¥X:è×ð?`\ñ]Fø?'"‡
a2?3µM·?ï¼p¸òÞ?[eä"Ó$²??­!Q?%æнÊáÈ?Õ²V+i;?ZÕ ŽVù™?ïb$oBzp?‹ÃéåÀ?S¦ø0Œ"?FŒ{ì
'?'‰—£2:3?ŠM=FsF?ï‹,Ìð;Å?Œ"K"?Rŀ™jº&?`ÇɔöR?ŠÜ§Ô»q?Š%¤
í§®?ع3?oÍNo'??irçϗ¸?h,£Î±t?£
kD
úS?'çü‡r?ï9w†…{ç?{>–yå°Z?Q±÷Ø&ù?DÏ-
V"«?—µï½G¾?{Iµñ^¡AGN4FGL J0308.4+0407?Þ[í!èiÀF@ûüe@ÌÀ9r×;»—ñÀ<K]Ìcñ@7žÐP?þ"°hè÷¦?²rÐWîï?³»ÀNÓç@Ôþ¢1î@
(Kù}°¿ïkL"=?ïôµ^œ£¿à}Ôvå9«¿ÛÊ÷_tp¿ã¸ÅÿS1Ö¿ÝI‡Þ[?—AGNrdg3FGL J0308.6+0408NGC 1218?ïùÂï~S?=+ɸ¸?æ2 ùæŒ?…|Ÿeq»?H`.®´ó?:È-¡à¾?ïۊ"êKõ?qÚÁÝ{Š×?@­X×[§?L·%J=Õ¤?p%Mϼf?nyŒ×"ù?ï°ºdNƒ?v¡Á$ZÐ?W{§p½Çg?^¢QmžP?€áò
åZd?u	"¥[Ú?ï©ÂçEÉä?^|‡;n^?Zxs݆ÿ?; òÊt½k?'@7©=¿<?\À"žø?ïòã9E8?L¨É÷²í?1×áÙ§¾?(@Úírê?UÕhú?HñݵuÀ¾?ï£jٛDó?‡areìü•?KæR"aùÍ?Y ~5s(?…fä}§ý^?…×ë¡¿¦ö?ïz.‹\H?ƒÿq/^
?aD8Ý¢Î?gú'Ro-ž?#n–¡ò£?'ʅD]?ïN¶S[C?vvŸaŒ9m?k#òpóϚ?V°V+?'Ä·?÷Û§?tO•å"êAGN4FGL J0309.0+1029?ìwôЙWwÀCÛ×Ûô‡ýÀ8ÜG©â¼ùÀ;¬éïóB'@e'æèW@Îy$¯ò?©çØýî¾ö?½Zç,IŠ
@´'\e[¤@ÕH©0տ؏ØÛMîö¿ÜUÝað_ú¿äEÂÖ[¿ç(àwúc¿çH©©µ¿æE»ãAGNfsrq3FGL J0309.0+1029PKS 0306+102?ï𠑅xû?N–ògn?(rèŠÚmV?FÂÕ"Á×?[°i`¤'?L©þ'w)?ï錬ÝTk?fӉfË?3ÿ•¥žB	?CM©ŠMÇ?có`2»V<?dn}ÄÎg?ï£YPJ½‹?~7hø>!?daË:ë'E?p($¯µVc?'9~-|?wà9²È"?ïõ«6`J?7¾^*­b?•³ãök7?["I?SP8{îJ7?6«Ë!θ¢?ïÞÆ(1¼*?c&}c?0¾
Ղ'2?&åÇD'w?o"eÕm?bô–¨>?ï¼Dˆ‰ë•?ˆÛ A¨?F8m¯å£ú?[dëõV¼?®öM?€@•/ËIh?ïyîøŠ"˜?"/.6w?i—7^üè±?r	ïqÚ9O?‹tmÓØ?'0gcîÛ?ïèk•½?RKˆ¦™Æ?)O>ÍUŒ?U-1#'?f‹ø}?Q"Vª×ZAGN4FGL J0309.4-4000?Û£$åÈÐÀM`_ö"FÀ;[­÷õoƒÀ<ÛÑ_ÄÖ@ ¤{jÚin?ûæ ÆI%
?ËÁ>â=ø?¼(ÝÄÁ»w?óܨ##ñ@ïkY?aj¿ï€x–Ó?ïý Ê]¿ÛD!=<v¿Øtâ*,#t¿åjÛuÜûï?³¦G":AGNbcuPKS 0307-402?ïïdÆöky?II??$ˆª—'¤t?º_Ùt/î?^¥\¶ÞO¶?GëÚ~fZœ?ïÙGÄK?rüµ™'£a?A•­‡}Y?I'"IÿK¸?qLIFÕX`?p¥{AQQ?ï'Q6‡H?p£
´'$ ?[
øWCK˜?_bneµzÄ?ˆ
SYÞ ?k žíjv?ï"À&©ÀŒ?f'îe1µÀ?Yïå
/ó?@«pQm?‡®xdDìý?eWú8Òñµ?ïâT 0«?ZYû*?7.P#®=w?)aU{v´¸?jŕï=¬ˆ?XӜŠeÐ9?ï–×Ç@Š£?‡ªl@™?QÍÂ~á¾?^%¶N*bY?ˆUíÛ*Ø?…ÈJp·Y:?ïTCj§­r?|¾ ¾–É?c‹%Ò;ev?hyMÕ?"-õh?w5,\RYö?îðRZ¯"?']{hþ‡Š?gžA»ê°?W¿ỳaÉ?ŸÕ–©S?'A©ô«AGN4FGL J0309.7-0745?îm&|ŸÀIükßL+RÀ:`ۋ¬q
À<b//˜t@Çñ²µI?ýï¥Å!á?ċ–€_Œ?·›ùñ9!?ñÀ£"î^î@Oá>Ê?îÂWþė¿ãW²8ÌÐ(¿ßT|Yó¿Ç˜iwÿk¿ë˜š`höd¿ U8»]dAGNbll3FGL J0309.5-0749NVSS J030943-074427?՗•?x Ø[Úôé?X¿#ĐË?K߯Oõ?…Ur´c°?vžV4D‹?￯å$KS?x\éš1?Q"g¸†?YDú.§½?{Ã&&¬—?sñ"Ù˜^?îàˆåRØ?'0•;iw8?êó×eE—?"ZÍ7&?šùinö±6?‹½vUIV?ï.{0«w?r7ø–‰º?n»õ‰Žo?Sc¼«S¿?–\âo{ä?p³
¾_?ïZ~ž
0?…‹Q:+á5?j‰þUŒÍ¤?c8T³øÛ?'^ìy¯Q8?'ϐ¹…¤?ïO¦êB²
?"Aè؜
è?aːgŽÖ?lNYšÊù?"Ñ°¤\
?'pDiDé?î@‹®ÒïY?˜v³×¯?ˆÑ?<Ðz?ˆXˆ4õޝ?¥ÂõA6áQ?"çóÞx_§?íúczñ\?‹[&Ç^?3¤AFC?o;Ôw}f?¬ßBq­?ˆêï*MdAGN4FGL J0309.9-6058¿³ÞaÀ¿lJÀHxj¹¦À8c9‰Ž‰›À;á"0ÉÌg@ýØ@N°œë]²?ŸŠz¨ùÅ?¹+
÷fÿ@‡¹E @¥K#É3¿¬Õ²_ÊQ.¿ãP;å‰\¿ç1tØÂú¿çÖÆz£¿é¹…\˲ñ¿ïïÉQIÉAGNfsrq3FGL J0309.9-6057PKS 0308-611?ïêb2éÑ?ZË£"?R÷0äÔt?Ež£œ—«?Y.£So$c?TS)TÛw&?ïÚe—V7?q,ÅJ??Z"Ò?EF-÷.~?pÛâ'´§?p,Hßø
¯?ï¤T£ùÍj?"–šPð©?j–ËÍ?xÔ&<
¥?€F±['|?€CWêÐí?ï÷¸wš<?4V4ƒ±j?/dSNÅLÖ?•V1áØ?IE3»?0hõµåÿî?ïÎÖ؜í??lÊ@Ìá?\^[Õé¬?S"ÜÀnõ?q|ü½nÍ¡?fÅÑ¤ây?ï _HºÙÛ?­ñlÈX?WßýÒïÁ?qóÈn-‹?"ì.)­D?ìËVi?ïŒ{†^(?…JŠíÕ?nÅt6c~?xîʤ"©O?…/Áj—C@?"oaM×?ïêþ¥·à?UR®)T?E3!—Y>?9Ü´hˆ–?`£8õW?Q½'Èq)ØAGN4FGL J0310.6-5017?îæÜ@ïD­ÀKmÖ¾¾QÀ:*Vˆ¢ÑQÀ<a€OE¸q@ yޓô"?üs$ºÊl?·•`ÏΉæ?©A|÷øI¨?òª—ƒ>äA@%"z£Š3¿à=¢wŽ­?î½:¾AÓuNÌí¨¿â©?ÿÊP¿¬yšÜËٙ¿çÝúºpªAGNbll3FGL J0310.4-50151RXS J031036.0-501615?ïøÇ¿z\?@sùy"Ū?Lâ#°lú?ڊ¹¿È?KãE_ο?>äÕÑyß?ïî&T06‡?fo^±‹Ë?*lá#ik?9S8<"?`2Ýü‹³}?dDX!·…?ïŠ_[ôâ?'÷‡"a6?SÕaKÂqº?aÉ
-©ÿ?Šÿ{ýzµ@?úûµHÆË?ïٓR¾Ïð?R1'tU?3"WáÂ? ‡ÞŠ?rDˆ]@ª?QÏJ¤í¡`?ïòþ%pŽ?K‡SèçD?1…¡¹¸?$õßìþñÌ?U»Ó}-ŽÂ?H¯óNj42?ïÏ}{çé?{_Š/h€?:ùõL7Y?LP"u¬LZ?vÅ¡ôÃØ?z¡Ññ)?ï4×ß¿1?ˆi³‡]U?V'˜ró>?Vùx6P~³?—üڄæò!?Œê–ƒ±ó$?ï¬Z+®…?je͛F€?A•x!¾í?6­†	¥E?ƒÐ'µÒ€?jaâAGN4FGL J0310.8-1041¿¿ LєݝÀJ¬7'MLºÀ:þˆ†KÞüÀ<‡]°µ?@ 8ä¥Üs?ÿë¯æâøˆ?Ç-fe§?ž¯×žŒón?؆|¥@¶…8?í¤.}ÁÌ¿¿é2þ'W¿ÅÞo¡ùd…¿è¯Þ|¸¿ÒÔó"õH¿Â.åE¿|ØAGNbcuPMN J0310-1037?ïžê÷Z??€­u'ܾZ?>wGE»nÅ?3"Ç?ÅÓ?‡Q‡ú8T€?€='ÄÐ?ï¶Öê™!¶?'[S'Çè?SdvÌ	?Y¤
53ûœ?°±zï/?zÂQVÞUÛ?ïX'×–p?¡Y‹rs•?\ÂìDP'Ë?]l
£Ž[i?"#vX Þ?~ÌÌ1~u¤?ëò,?idj˖e?:áŒG?&º½[?
<~‹v@?iSڊ](?ïjW>p?'Ñ¡ÝZő?Q_ò™'Z?GHO²×d?üµó—fä?'nGîLð?ïcê[p?'E?äÂC?YoóeÃ?gtÈwA?'‹¾4œ?H"÷?î'ãU‹ˆñ?"$ªxFà%?e—qœ]—Ø?g@î™è?¥xSŠ×äø?"©ÿ$Ü?îx"¿ü@?‹5ñƯ»ë?P"MÝÕôï?E`ǃa¸2?§ò•*Þ¡?‹L©¯nö‹AGN4FGL J0310.9-3458¿åþVèoÀM¤N¤¨ÁUÀ;cârPÀ<æTe²â@@D[GNs+?ýÆ,Ÿ›;Z?Õ:ý Ë?ÀáŸlÂK?é9¯ž¾œˆ?ù-‰Ó¨ß?ïüà[
‡¿â˜¹Z)A¿â‹Y?aiÒ¿Òɧ~^«¿ëÒ/]•?Ջ÷-âAGNbcuGALEXASC J031057.27-350033.4?ï¿ïªÙn?¥+Öêó?Q¥¸?ilƒ(ñhF?à#é)©æ?¤|æ`•Ã«?ï­FÈøh?ØU㪓v?_ŒhrËõš?dòy£:ÈJ?€¼ÀÃZ¯b?|
ÜSÈé?îö:µÄ®¬?'""†_"?sS½f 
?v;
6½2þ?œcº?~d?MÍ'
'ò?￳+2€?vÉQ"ýù?i[ÂUž?PÒí[ƒä?™ÆænT?uÐ}w?ï3ÿPO<?'¼Ö;‰¹•?^ñYz´Ý?Z•FÎ3?—'jtm.?ø'qÉ?ï'±HљÕ?–özÓØE+?k<qÉ9¦?sÞdçË©?—¢H³°Ã˜?"ÉQGdP^?îbη'.ð?˜ŸšÏ—¸?xo%TàÆl?|ðô±"¨4?¦Å/Ù
W>?–žý®Ú¶?í0×/ɔ?"G]ß?w
Ó¿èˆI?l¸oŸT}?²
œ	†GŸ?'³;¦,!AGN4FGL J0310.9+3815?ïÂÿ•»­ZÀ0ëã}é9ëÀ:
ZÊPñŠÀ<:"^žñÈ@0z·\Ç@qg#$È6?¿íQ҅že?¹Ç}W™™ï?øÒÅjüZ@äl$ko:?ïà«ÁºJ¿ç4éKˆ"¿ã â-‡!È¿á³/'N¤S¿ío
D& ~¿ï×ó;Ì^éAGNfsrq3FGL J0310.8+3814B3 0307+380?ï‰BL¼ØI?'¡þî›B?[‰ÆÏt×?QSˆP6M?Š>Lrȕ?&ƒþÎç?ﶥ¬U±?+FPÝ?Zf^??bþDñæ7?~%ÐHÖ&I?{ësjìï?ï]$ÌPY?‡¥	'º} ?w'ÓFÏe?}÷ëS‰‹£?#ø¢£
?¨cÐû«Á?ï)ŠŸÎƒ?q¯¨¤$?2ˆR^h?`^¸D?'5gßÅõY?j3»²ë¹?îõ¬Çô Ñ?"9ˆ‰gL‰?r}Idw¢?j×ù+Ž+?œ««:ô?'ÜB&9Qe?ï2b‹:†9?šeôM/¸É?qäz¡-x?'·è½'Òº?•s5|š¢‡?"~'ð¯Ã?~)Èô?"í¸ûj·1?"ñV_?"×mk'"*?žq'Œ'dJ?FA±9ï?íá]W?ŠœŒùoœ?•êΦ§Û7?züíi¸õç?¦ôƹRëŒ?"›¿%Ô¬¾AGN4FGL J0311.2+6856¿ïË1½Dø
@"͒·þ¯À:¿ޱџÀ<2$fÖ@ ¯ø
é(?û‰Uê`o?ÒEÇ_zŽç?ѝbœ,p÷?û-%g˜•Ž@ æõ—ò%¿ÉÞºu‡@§?ë­ÃAޜ®¿âò¡r«ï¿Ùˆ›dÊÚÚ¿æ$ü=s¿Þ"˜±<MŽAGNbcuNVSS J031111+685610?íԁc0À¬?¢VÝ®Á²?gÁÛ\P› ?ZF!çM?°æ
òˆ"?¢¦ è7I?ëé_×ñˆ?¸ÑƒÊY¾?yà\
×_÷?}Òòö–Ÿ?¿û"›/Ç?¸6ÞQÀ£?íww'K?ç?œß"/[) ?"÷ÄaZ?€nf¯?±Á‡Ëƒ$!?ši4áƒõ?íôú€5?‰z=ó>|?ƒÇÉ>4"?eû-É??µg_ëC?ˆÇ£Œzç?éÅlE?·wޅrJi?€ª
º
½?qgMG™?Çë+®?Õ?·&Uy£å?ç8ùÈж3?È]ª;c"‹?‰k ˬ°0?'š¸š¿2?гgå±9?Çò~]å¹?émØfš$?¬Å£ƒ˜Ê?•'*pu?Œ £‰h'<?ǖ[@î\¿?ªé˜{¯Ç?éÇ©w]/?¡Á"ÇhKþ?^ÿEÄ%!?{V̄ñH…?ÉÁp ,#?¡î˜Ž&ª×AGN4FGL J0311.5-4402¿×{ŒSòÊÀLž¡3ßÀ;e'Ýãu†À<ãñx7@YvT3ˆ@pµ'-lJ?Âϼ<0Þ¿©in"?åkÛ@#œ@,¶ùPäI?ëËw͖÷(?í+¡~•\H¿ãÝløPß¿ïÿ ÿ¿h`?ïý''N#z¿à¶Y"±ðAGNbcuGALEXASC J031103.24-440227.8?ïî×[œ	?W}·?¹ª¹?-#3ÎýÉ?1@Øx?^¬â¯^¾,?Uz:¦hÊ?ï×ÞáwSÊ?zä94…ìß?EB'B-² ?YQ''6À?qh=3ÆÜ?uÕÓm8/L?îÞÆ
ã9î?•9å»}?r˜Åäô1{?}suCR(?ŸЋØ?"·¹Ùïº?ïõ5'š2,?EiÇm2 >ü™çê*É?åj¦a²?U"vhºC%?DØ¥—¥®?ïâªó;Ôö?cýçvB8Ì?=õ:ÇI?9½7ª5ã?i–e®ÛÆ?b_ïj5ÇÆ?ï¥?•í?Œ f,"Ök?KGCÁ)l?]ŽX_Aˆ?…vBáØÌ?Š&8ƒ<%™?íÿTΦ?›8°fQ?{vÛ3Vìc? ½ƒèZ,?¬¡VJ"˜?šm%ޑh?ïÖÒo׆î?iƒƒy]?‡^™`?#9PD6û?t(ªœŠàz?hۊ懍ÅAGN4FGL J0311.6+4134¿õ.&LúÀ,ô{gkÀ;z/—@À< !úü‹@!mˆô…Î?úO}¶åû?ÙFf@Ѭ[?Õ,ÅÛÁÝ0?ùoz^Ù@g"#ìÞ¿Ñ5®ÃLpq¿çæf0¶1¿ìNÚX¦ŠC?º#Rë__¿èe;ÞÓ_Ž¿µ 8š%Z­AGNbcuB3 0308+413?ï¹Ô;ùLÕ?~D±6K	?LJ6©B"?Aô½×?Œ¡'ýN?}bßÁ7?ï;T¢Í'™?¥+È0µôQ?eq¦'€Ž^?mOø\èÏ:?•ç6Ù¦'
?¤ª+´`[?îÝs¸€Ü×?"kâp/åa?lœÝ|å‡B?muª¼U«? ^ö£"v?'ýw6á?îè"` Ò?'Ò''Ÿ¹?_xƘ†ÆB?OÓYT5~¹? zùBè1?'ˆȾĥ?ïx~•Ëóx?†¥Ô8ljÑ?^Õz¶ž?Wï<ˆeî?ŽßÐEäL?…R#ó¬ü?î5?¢Ø2?¹¨™ëèµ¥?s+ŒÖQ­µ?ŽHœ{÷W?ªIZfþ¼´?¸ÿÁï ¢§?î)ŒVm¨ƒ?šÀ8ƒ˜ë
?p¦S[²±U?tZ]^óX?«Rp+µ[.?št[¹½?ì;A˜`ñ?£nã$·v?t'~I(ÿ?q|ÕÛj§š?¼ã×%Á0?¢Ñ1£u—ZAGN4FGL J0312.4-3221?הª˜*¿ØÀM‹ºÜ	€²À;ylÛM™À<÷#a	/@Þóú?üã¥Áƍ?ÛæŸê$Ì?Ñä"''?úNãx	üÙ@ía½ª?ï±ÊÛ[¿Ñü×V"ŠŒ¿å¡@Aº¿Ì!8	ã¿è)Âbæ¿ðAGNbcuNVSS J031234-322315?ïä2Q‹ãÎ?`i˄#ï?AÄ$h ±ä?5Ù<Së?g\¥O^Ò¾?\ïR…>´?ïÄ$Þq;?xÆ¥¯g7M?Q¥?ßýÍ¿?ZY‰ê?y"@åúûq?t'±ãåà?ïZ-ÁëX?'š:2f¾«?rŠ9À÷o?y+.°VDf?¹Z)AB?|Qs¥À¹?ï†õh*'?im?CmÛ(?`"Æw#r(?L-Å¢Õ÷º?ŠtVª`Û?g<dÁ"ð?ïËóÈSN?s'ðk
"?Qþ¶Cmº?L'#_ÜhA?u†nT؅¤?q%Ü:*'?ïnQ+c'?Yl.±¬&?\'½–=?nGq‰%GS?mº…±â?‹»°Fþ?ïŽ\,Y?ŠDË›I(?u\¨VÞ¥?zòzÃÃ?š}÷al4?†Ù¯ú¨)	?îàe'?"ÓUºã"?f€e¿B7Â?aŸâ~§à5? '¨uȈ?")¸\YõAGN4FGL J0312.5-2221?Ð?	)8LfÀLÛƒjƒ,À:8†-¬
µÀ<bãv\}¯@ N™@-m?ú®4Ʊ)Ù?Àtv‰õÛ?ÅF×)òíž@I¢ÿsé@Üwý½…‡?ïÿì´É È¿Ýq ~¥¢f¿°¸'Ï&ï-¿×⛠}.¿ÜXJy¡¿ìy&\‹RAGNbll3FGL J0312.7-2222NVSS J031235-222118?ïÆN3ûÁ=?qÐq$a?P=óla¢K?EîO4Y
Ý?xÉiAi?o´ÁYså?ïÉÝ7dV}?uÇ÷%Û?Lœö©"]ê?Pe{ú^@?w}ÅZï$?s¼ÎÍ?îܹ¸aË?"	‡ûñÚ?iÞ>Q°ßú?oz' )eà? š }#[?"X"%"??îÉ|)Ÿ?v«¶Iw+?mr¢RÞpÏ?O'PM|œ…?¡'ú]à£?uy0@ˆ?ïqÕÑЏ?"
äÓ³T®?m,ný?fF^ñ>|?Œo/Hç?€»‡?ïmµõ'5D?–Ç
bl›?`K1úF?fµƒ]Ù¬/?FWé{"C?ŽqÓàoõd?íÖOÈȹË?›ÈűC'#?~@ϹËB?šµÝp?®É[Tï®j?šŽÇúBC?íC-÷µ×?ËÅðøk°?zã|­uҔ?f®ÿS?´8XxFu¡?-¨JZ˜ÝAGN4FGL J0312.8+0134¿ët³¥Ö¶'ÀF½ke©¨À9ƺNEqÀ<(ó"Çz}@‹‹«sÄ@-òˆH?ºùµkŒ&?¶U¶ë¹÷Þ?ù˚¥—Õ@»I)"£æ?ï͐â:ó¿Ñ!DÚ$¤¿åMú>ŸøÙ¿ããe€À¿äéëÁ"š¿ðAGNfsrq3FGL J0312.7+0133PKS 0310+013?ïòÆ­4<Y?GÀ›¶²ô?'µúñ‰Ë?¾/kës‡?W{ædÕ@?EñÔoEQ7?ïçVGקi?há*¬ðÇ%?3'ÃJÀ?A¹€ü' ?fGeœ _à?fŠI3ˆ?裂)G?t"DÅRÂ1?`îÃze7A?e èMžÓÇ?'G™Ô S?pԑxÌ8?ïÙß´ïÉ?OÞ»‡ä*?@š›e§¸#?$47 Ò?püÒeË[h?N×»½Lö¥?ï隰ÅÛ?UÊëšq?7Ý̪×X?,U&.—?ci•Ú4n?Sؤ«ß?ï´"xi·î?ƒM±È?Cü¥ë?Så灀1Œ?· 5Úh?'*"š2‹?ïežÙ?Ê"†¬"Ý?jæS'îi‰?iùÜ®ûÙ:?ÞåÔÏs?­6«œm?ïšløHH?n•yb»5Ê?VҒüGìÚ?BÏÅâËÁå?†Šoˆ¨?lÝûˆ ò¯AGN4FGL J0312.9+3614¿¥'Ù•†Z:À2i¶°_¯À:ieõ'_À<?
 ë2@ žôÄ7§â?ýYÞ7X\?¸Ã…¦G§ß?«I­âÀ˜Ñ?óÚE[Sã­@±(Íÿ|Í¿ïýgß?ïãϝ·‹r¿ÈqMàˆ–g¿Û±dÜ£"¿äeÜÓ«
¿ÃÏéŒÌAGNbll3FGL J0312.7+3613V Zw 326?ïÝÒ7^ªÊ?aݒ«µn@??"LyÙ÷_?2s˜ÛQ?É?n=?*×&ê?`+i›ë$œ?ïÐN·s[?uï}—Sšç?Lq~»¸/?Ue®Å4?tJtjýy9?r3;›¸á?ïf6]èœ?–dPL¡¬?h.?¾9í?j¼ÛÜêÞ?7.>C?}©‡4Q•C?¨"¡L?vYM|÷(Á?}•›g4ü'?YûáB¾¬$? ¤b
F°?t:«ò<–?ï±k†Ð'ÿ?qì¼ìƒñ?UŒ7˜Šk?H֋®ãì?€ó—Kg…Á?p5}6HÓº?ïwǤï¹?˜ ‰«?aŸ"îžg?pØ®¬û?¦2ô]"?&(Ǝ=r?îòO.Lªº?ˆ³.¸q˜k?qéa

Š½?nx§[LŸ?;Áù¿\?†cà5;£?í6Ú÷KÀ7?©-:"´)?Ž
F–A"X?uÅõ³ñí—?²‡ßsµ²¾?ŽµCq®hëAGN4FGL J0312.9+4119?՝qEùšœÀ,7A¿½ð'À:7"¶
m§À;
ñû@§Ï"þ)f@+¹!]¹?»O'ÿƒð¿¿W4ð!»'@f"f\Uk@	¼óíx¿ØÔDRÈû¿Ëcòl¿Áj¢
Vp$¿é~0O‹Y¿ÅV1ûOÂ
¿ðAGNrdgB3 0309+411B?ïÚ®Ul?°ÊYÁ|?a`»¸òŠ*?u7‡Ÿé	?›ø'ÊÞ»+?®æ"$8K?Æßwõ? µå'f[?gQ®PkI?y'9Y+*?‰ƒb¥°‹ö?¾¸8Ë`'?èYšäó4?± ]@Î?¢cW:¿è?šãQÄÈl?ÊÅKÌ?°IPtWƒ?ì­÷Ók?¦móuôr?Oû:¼ìö?I–­³>f?¿™ÏcCá?¦QnþA€?îéu˜55?°`RʗS?p¹èi|?|²é¸r"?žË^‹ò)7?¯·öë&?îÜ©=wJ?°`Új­
Ž?{">×ËÀ?'5üÁÛM?¥Ö~$¿?¬÷¡›Gxø?çý;fÕÄe?°Œ+™å-'?¦"ãäÿ9*?šCk?ʂYk×£?®'¨¼µ?åYÁ:ـö?ÀUúæï€?j"Xç?p‹Ê͑?Õu…›¾k?ÀJ7—Ø	¨AGN4FGL J0313.0+0229¿Àgì£VܱÀFhfýe
À:×+•°À<1œñ<îž@•<F,_/?þŸ°i¿·;?ÜØÄ|Ç%ï?Þùà@ÇñF?ûë ªšrÝ@áão{ë?Ûh $ã1¿ì;P8&¸¿ÝdgE‹%¿èIŽ;Tj¿ïÿÌÔY‰¿ïÿþÐñAGNbcuTXS 0310+022?ï#pdøJ?µõ³élŽË?j¥¢ÊÆfo?‡h6뼋"?˜=H{hü?³ÝôÊ(£?ï|œ¬&A¼?‰R½'Ça?hNÄÚƦ?p+ärKp?ŠÅM7Òey?ƒëS´~À"?íêH€tÉ?œÙ‰CØi?šl€½ÇÏ¢?'êZ܂gó?¤%>‡\ý?"ߎ¿w®ö?îSšóêQ?‡áài¾ˆÝ?e}õäÊÃ?Põã.&›®?©vVó|šø?‡{Ý=´¸?îñµó|å?˜7Bð6?xa·	&ÿM?vQq	ÌX?›°ïÅ¡ê‰?•ÂêàXü¹?î¯í{÷zÔ?¢j¦ýw"?x€/+æ߅?†Qp瓨?¡ñ"WóÐÕ?•ÙrVòq?ìʹ˛–Á?£8{Ï1À'?ž(§‹l&¼?"±Ç@yuj?²/À¶3Æ? Y^<·›?ìR> wæ? O¶Òˆ¥5?hþn.ؗÉ?bLO´R=t?¼¦ˆÂÔ? '|呑NAGN4FGL J0314.3+0620¿Êì+"4¥ÀDñLìAÝÀ:\¶wòÀ<:Š:N@ Ώՠ…ò?ün 9[ka?Ɩœúw*?½[$À?ôdõgö‰_?÷Տ;qÆ¿±§Ð(Q¿ê^ǀ݋¿Ø oA{P¿ÉWX×\»¿äíÑÅZ¿Õê€Ý
1²AGNbllNVSS J031423+061955?ïYmÿÚ?‹Ð`Û+?>û´ˆ´Î?0¾ú÷4ƒÛ?"c?  i?Šâ×Òěk?ï`Bæ.¢?‰ID°E®?n%xyR@.?p7ç9ýÕ?2ô(nN¶?ƒýöݹÑj?ï¸qÃ^1?Šÿ¡Rø*?gœ)cË?dΣU@?™Ul¦Ãä÷?Š‰œÂx?ë‰
"Ì;`?"ÃÐ%?ˆåh'.?k‰7*|?ÀS¹³ä?"¹âÍ/Â?î•9µÙ@N?—ûl×ˁ¿?SÎ؜5¬?G¤ûàkW?¦
íـÈ?—Ÿ$År•"?îF
Í6îÃ?¤Ë.}q
í?€‹ރG
?‰8Ç&	?§|a0ŽÁŽ?¡íX7Ãs"?î)=æë\?˜7Ž€™"ý?t­5˜S?pª"Xß	¦?ªÖzáÍ®Ø?—6λgß2?åÊDŒt
?¦c2£&œ?˜M®•œb`?ƒo}×h?Òæ›þ¬K?¦ ¸rêÝAGN4FGL J0314.3-5103?í=÷ßõôcÀJü©iuÍÀ9¨²ã»-À<XKƒÂ@úñw§Š@u_þmY?°S	<i½´?¤-?SR'?õ²`Š"Rà@ˆýµLþ`?ïè'á´,¿â±Ÿµ<O¿âtô3C#k¿Ý¸ãÁ…ñÇ¿âÖÑ"qïÜ¿Þû:]ôÒÐAGNbll3FGL J0314.3-5103PMN J0314-5104?ï÷¹Œ "<??Y,î¼mŒ? Žñ|†ò¤?	˜d#Îß?Löv6–¢?<ý±]íä?ïé,bè
?i1#Í[[O?2¥Íù×m?AKºc—æ?d¨#D±\?f\t'¡¤g?ïÁa"¡²?o‰£Ÿ…U?Rå3}*
?[!ÕVúÞ¼?zÀ'wÐ,d?l×»­d?ïÓ2	Æ?P"¢¦Ý–î?OþÖ\
É?0怯=Fê?rg:՞—'?M¾"Låá?ïñ2–ÄìÈ?Mн˜?3ÏϛxÆg?$ß÷Çã
ö?X¦Þ'|ª?I'+ä÷™?ïÂE¯Yè?~Ù>Í&®$?@˜è|C?QQcQãgc?|Ê,©Q?|mæyÒm
?ï•?y+~Î?€0ÝÓ8Vs?Yu¬­ÝU?VöpÑÄ?‡l)³}|?"ÃëI‰?ï•fêDØ?n†ˆyÇ{Y?cÄbàñ?L{z><£X?…ôõ,^Ð?kØË;ܓAGN4FGL J0314.6-6549?ï
?§	ï˜ÀF¯mÚÎîÀ:ʘòª¬çÀ<¡öé	:@1ª‰€ò¯@')Àê?¾"ÛÍÐf¿—àõ@?ƒ?ÕÇ,#õR¨?üêõçÎ/ù?í™ö`ÄæÏ¿æÞÕþ¤¶-¿æ·é{Y<²¿åK¢•ÁÅ¿Úaf'–¿ïþÊ-ëÌAGNfsrqPKS 0313-660?ïÝòêÌDÅ?d³§_Étï?GVÈÐV¿C?<æ€æ}e?l7bûug?b'•U?ï°v_­ºŽ?|Ë^Oy	‹?UäÉQšâÒ?\÷U ¿'?%Î䆪7?wúµ™ÑŒ?ïX*á!ê?€™Ø%ìß?mø†áÉp?nÂiàÜ?'Y¤Ò€í†?{¬r	•Ô‹?{þÿ?d3!øp½?cîKCÉ!?K"6…çf?"X<KǓý?bŽ(ÕØ(?ﯛ·^¯?w˜©4ON?[QÖÜÐ
ÿ?Sêޑ¸}?€®×UQ?2?u å PÀ~?ïºÝ$øw?•q¹2½Í?cҒî1†î?nwyAü?™®Qÿª"H?"Ä0þaH?îÚçÓA
Å?‹ºL'Üùý?yRåïZµ?vLJé"ª?žNL$û©?‡åæƕr?îÆT+='?ƒ@´í/]Y?€lašª0Û?paùî»®p?žÿMÕ*QS? ¤Ÿ4ú»AGN4FGL J0315.4-2643?èCÖD"wWÀMYÝÁç–À;M¶Šk(À<¼½qåöi@!
K^"E?ú¢Ë;Óå?Él'Ê !É?Ǎè5ˆøâ?þD*Lä'@žq-êžð¿ïû—?ø¡¿ÝùV-3>ò?ïùÄýuŒ¿áaÏ}×Z¿àž+ϑ£+¿ãåªê#õ©AGNbcuNVSS J031527-264400?ïߖž+`?^ÿ(:@ù†?A¶<l"–?4þçÍ¢#?kümÜmw?[¥[dlˌ?ïÀUsW™"?~¹hD¬U?PíxbkÝ?X¨h»<˜î?{™èBwài?zT#èm_P?ïmüç`¨?~TòE6PÙ?aøÖ?Z*O^2øg?cù'@?}SìM‡þ€?
'?Þ"m¼¾±?`
$Ø7Ë/?S¾]WxÔ©?£Md^d¿f?–Z\ÞK|?ïÀœV§z?oµÊ–÷?T§D4ßÇ?ZVµRŒ†¸?zˆži5?kš5?ïbíú³©ª?˜$µÛ³^V?[8Ú½?d3ŠÀf£ª?'éM/4€M?—è}ðU?ïKs¾5'?†sÑdàJ?kÉsµZ"?pòД?š=c¢m?…9
~,W?íËSPý?W–,R˜?j@ë°¥=S?iZ9:ûƒ?¶·ž	½Yl?œÕ"œAGN4FGL J0315.5+4231?»"Ǖ«MvÀ)¨Ût´À;lŠŸ*ÓÀ<—!Áçã@!rg‹T‡l?ôû…—"¤?ÜýŸ—Šv?Ý×(›T¯°?ø›ÌyÁ@A:¤Ék¿à>ÀÕó'¿å*øf®ŠÂ¿ê­Ù!nå'?µuc.xŽ\¿ãâÌ'ª¿äµðè5AGNbcuNVSS J031527+423249?ïÚ5ã^+&?gô6(0?AƘ>#PÃ?9/º¡9y?p¬;8¹z£?eº
ª_Xæ?ïázG³?ªe2À¹Çv?\E¼®aÉ¿?ga˶õ˜?›_tï;Ë?ª*
zðj?ï7m)¤?'½v;È7z?n•ã¶c?mÅ+>õ?›æUþÇî,?'P½‹%'?îÁðq'ñ?'­D-7Ž?U,÷ÓêÛ?JæÁb%$M?£7—ù‰Ø×?'"76ý]?7h½H?uW0Š$?R'xóѤ?J	.²"ôß?}Úáà÷¦?sÎB6s?íªkXp?½ÀE«8†?rRZ{›?u¥†}VD?±‹B8À®	?¼öȞ¿É.?îK}Â×C?œ—ÈqP?q¡s[D$?rìÙa?©õpÓÿP?œ*òGÌC?ìš.t)? Ô:¡³æÄ?aEXĦ.q?ajr·ÇõÕ?º¤a–vQ? ®+£AGN4FGL J0315.9-1033?æOÓï£3ÀJŒCoÁYÀ9‰ÞNÕP)À<8€eëí$@#Pn'i§@tpë$¦¨?± $"I+?µÈNŸ¥m@uûdÌ'@CîÅ&?°È`VìÕ¿á9äþú2¿è𯮯¿äŒ <Àü¿é/–Ð<¿ïñneZÎAGNfsrq3FGL J0315.5-1026PKS 0313-107?ï÷0
|?@ÁÚ»þ	²?)¯Ünÿÿ?oõ9!]˜?LÒü'¤@?>K¹2~‡?ïêìx"Õ?h‰ª=Ì®`?2nùõ®Ã?@ÔÏÔB?bÆIܶ…?eU""y?ï¿ù
â/¤?kA<®?TÈÿQö??ÈG¯,`?zü†Ö¢ÔK?j{쭎S?ïôÏ2¶>I?6YYâ×Ý%?1¡þb"Ã?¨N¾î#R?QùÆÈVg?3ðtD>?ïñQ<Íw?Må¶'ðÌ?6æ°$JÆ?)¢Ð%BÇ?W£õõe?Kœ³|J•÷?ïÄ÷©ç'?€–`¿´fŸ?A"0o?SŠÒñ§?{½áÅÕÔ2?~»ôÃ?Òû?vHÚW®v?`¬M±ë?QÌZKyõÀ?‡¨E=}¸2?tpÑé+}?ïä@T;?Sí2?¼²9?HÄ XŽõˆ?8ÇV¥Á"@?eµ·S‰*?Pz¥¦UßBAGN4FGL J0316.0-5626?ŸeC¦äÀI€Ç`|À;"¶Ò"mÀ=½‹ç)@ .ð%ä?õe¯ò¡r¬?ä=n q¥	?ä:ß%"å@÷üü?@•Æ1}%›¿â"ií£ù¿áß
váí¿ã‰Â@׶‹¿Êùá'çQ¿â©9êÝY¿ïÿÿ&¦³AGNbcu1RXS J031613.4-562545?ïæ_ª¬^?X×{H>ì?KVð¯–??säÔÈã…?bÚ'_¿M?T\/*5ð¿?ï«ÊÎð¾o?¹Škþ?[&5"f|J?b–6•—Ç'?¨…­ñð¿?}WóG
Y?ïÙº›?ŒY…­SŠÂ?zºPԜå?Zv.2ªç?•VHQ¡Š?‡åŸz°Õˆ?ïX—R0hA?s*;a°Â&?SbN'o¤?Gm•[Ó¯¥?"¶ðØÊÐ×?rl,;+Öò?ïÒ%¤PÃ?hxÖ¾°°?]HÅýô¹?U€	"-´?o5ø¬ÆêW?bµ`½Õ6?ï%@‡ÀºV?›KÊ¢´?e»W¸j'?tò§Q™I?˜ " uê?˜'Âã¨?îÂ÷¬–Ä?"ªVÊï?ziQA*§?}¸¹¿.Í? '`ûŠ?',¨–b›?îq½&çup?–áì4?N?Ug§^Ÿ6Ø?]çÃÿaà?¨8ðW-Ï?4¶E×
AGN4FGL J0316.2-6437?×ìéâԘÀG|"µÜÆÀ9êHX^eçÀ<3Ð&ô`@fyɹå?ùpÃLŠÆ?·N[ؘÝÝ?½û&Qxm¥@	›ü"$íö@ƒýLŒx¿ÒLŽ£ò8¿£‰9¥H­¿®·}bßÑÀ¿ÒŠ4¸Œ¤¿áqÊi¿×ÙFWÓ%¬AGNbll3FGL J0316.2-6436SUMSS J031614-643732?ïÔó~ߦf?­')ônÊ?UWÍÀÁgp?Îð|Î?p0M-ºã=?^zï)*6?Xo?r?zb¡?P.ù"¸R§?Töß1^µÙ?}˜
‰$H?w;D24´«?ï[Uɋ#à?"<'j½ˆî?r»Üô'ÿž?tˆK¾pì?ÌŸ(Å^(?'êsx?îѱkë?|Fhÿd?j5 ßTü?K¤ñMÆ%?¡AÚöû?{{Ïs?Ÿp²?Œ¿0cu³?o`ˆn_—?Š²{ÝÖ?ƒÎ?ÿw…?s•«o"VP?ï}G,? ò^»êU?jPÝm¤ã@?ö+»çú?˜ò4ªŠ	?žmç]HÏ?î}/ÊË?–5šú>`h?ƒÒ掷4×?ƒåcõ+?£8Tü£Øv?'T>""K?í¡}Ubªg?"O0Öâ3?u¯üŸîÕ?a½ß…÷OQ?±™•\€Ü?"f'2f2AGN4FGL J0316.2+0905¿è¤vfPRÀCɤi×4/À8¹g«
fÀ;«ÇQbÉ@®Ô²?ýЕÊ@r?©`¢G'Ý?®õ|æ§â@¸G¢'v@9Äè§É³?ïöæç*F%¿ÙÐwœn¶¿Ý©·ôÎs–¿ÚCyÒSõK¿àðíޕL-¿àí¯e³¹AGNbll3FGL J0316.1+0904GB6 J0316+0904?ïì8±]–Å?Uâ.œj@P?'·'ß?"Ä:4Ý?bKÝ-×ün?TÔĦÚ=,?ïÚw‰yç?rêyp°G€?@okûØ$X?I3s ¦'?p¶ˆ"²â2?pà´àÅƪ?¹<!?€ÞFÍéà2?c0Ëôèy@?n֚Õӌ}?†Ä·×ñd?{%#×ߪ?ï1å¦ô‡7?se£ù:K?bJ†ò'?Dƒ˜®ÚZ?—yúG"a%?rvüú§§€?ïÖþ1§J?kC‹)rÁ?=ÎO=J<Ã?5–­ÌÎLv?r¤)V4È?išq˜º?ïŠ}¥ê'?‰	Ÿö[å¥?Q¿ËSõ?^ôs?‹G§'"zå?‡aÂu'yr?ïMf+,?‹<"¨?k0ï‰ð}?rϊéfÚ)?'÷uEf"?‰y_Wøf8?îC½'gé?'"m×ã›	?u<²‹tÕ?_grA]?«Ä-åîQ?J(SltÚAGN4FGL J0316.2-2608?îYώ6þ´ÀLݍ%íÐSÀ9ÇøåY‹À<6@<H†@…[f=r?ücZ'ó+?µ\ÿ	Šî?¹s 
Ìã@Ì|Dôü—@PhÖ-H¹?Úöóý=Wú?Ïk>¬¿áŒY	†'¿Ð娶m¿äÕ\Rç-¡¿Ù›2Ál"AGNbll3FGL J0316.1-2611RBS 0405?ïæäà¥?TÌwŽ>3"?<-WT àÙ?.7f¤Ûmë?fvpÀù''?R­£üCé×?ï¼ÑÇÞPƒ?š°&@ï?Y"ß¿Ÿèë?cv9 "Á_?{NdÁ¸u?{•Ž7ã?ïfþ­"@$?|ÞYÐH‡Ï?k^™;ÆlÆ?kºý4{47?h®wô™ ?w°"î?î«uQeÎ;?yŽÜ՘?'øYn…–?cìŸ_0.? Š£Ð‡Êî?u–•rÊ?ïÊðÑ[II?fBôºû	?U7Ë¿úµø?IœŸ"Ìš{?u9¤_œýå?bq¡œ·*?ï ž—Éúy?›É¾X€ø?u5£Š¨?"¡'ŠàŠ?–žçd½>Æ?–<þÍØ?îÅô&5§_?Žº_ݗ<¡?}¿€3Æç?x;­\Çd¯?ŸÑ›1¬òÓ?ŠMV¥<?í&ԕ""?'»äCÀ?"ƒq>O©³?} ÷Čª?±è
:v?Ž/‰^Ê!AGN4FGL J0316.8+4120?ê]X,´5tÀ+g0«¼²À:z®Žd•À<	›h¦²‡@"YBI-Æ?ý[8jª˜Å?È=º ¥Q‰?¾ú|2€†@Pÿ}¤§?ç:V[Vh¿íœý
y¿ÙBW}ë=P¿åqÏ ¼£Š¿ØÑN;Í5¨¿Ð¸
ãmx)AGNRDG3FGL J0316.6+4119IC 310?ï;àPÅÕ?šŽ˜';4?;=Ñ7"?;}|jW2?˜¥g™i?šOW½<r2?ï<:ÙÎE¦?° QËx?Y‡@/"?la:Ë·‡Ä?–à3Ã¬@?¯ қ߻?ís0çS‹Ã?£þ·©Å¤?[œAxÖ?d€ž^B)?³ø½Ru2?£#0,¥?îBg²Rr?'Šw—ÛQ?V¦1Ú"Ø?A~yWž'±?«$SJĎ)?'™³q'Oº?îZà'Á'?­Ò·1)ú˜?Lýø
«É?GÇI‡]ÙÜ?©ÝþõÕ3í?­—ï4%­?îœÙ…þîC?·MFÀê҂?_a½Y@Š?u''9·%?¥7Y·ÆC?¶óP6Ù?ë/^uS?¬?þºE?k>ÎßL?rÀm?ÂÖÖGí ø?¬®ÚbPq?êA^š=Ð?°ŽÚm?na;Ì
b`?dí–ĸ±?Ɓ¨há¸?°ÆY‹aAGN4FGL J0316.9-0625?ïSCu÷¢ÀHÞìAÝ"À;Ÿ†B¤ÀÀ<©ÓåjS@ "DðIÿ}?ü,?ùë	?ÑA ^Y҄?¿¬œU¶•Ô?íÞ½ý&1@aÒ"ø¿äEå½_¿ë5ßàл¿Ñ«±EX¿ÝÒéý	U"¿à»ùu¢CŒ¿×]cß#'AGNbcuPMN J0317-0623?ïñ—¯tÅ?H¶;³íaå?#ðÑ·<?*'ù="·?Za̛s[?GšÈ!¯îq?ïÈ«Q…Œ?uȂ<¿#Æ?FÕ¤v.@?QsBå?yõêâfY?s/"ˆ±ÁŽ?ï"ÏÅЄ<?pܶâF?VMzMNô?GžyYB+"?Œ_Nñ´÷?nâèñO¨?ï'6»ö?d˜_iëS½?Aº'Ý°Ë?(D"=CÊ
?Š_Pûù"³?dGËùl­È?ïàÀùɞß?aBR"9Á?5Ò'j‡üú?*óìv`Y‡?l"ÁX—÷#?`ªüPœT?ïoO†a??‹ªRÁœV³?VýœŠÿÌ?dŽ±
œ?¯|Mç0?‰Z9ú{?ï+cGÅ]å?2­Çæîh?[\‡àÄ
?IZ…Ü`Ÿ‰?˜ÝΊŽ¥$?€»X ÷O?î×Û^¸?ƒêß_‰?P'@ùB?C=•jã¬c?¢F˜`?ƒÏ@£ÊzAGN4FGL J0317.7-2804¿ïS©Ý€ñyÀLÚ'¿aª?À;ü/çCÀ<Þè	i5N@A`[	ø@þãþA¹ß?Ótá¾ÌY
?§ÂIÇI?Êê›ê¬±¤@pM
ú¿y¿ã-Æèl¿Ý¢}ÃÐ#ï¿çòbo¶Ç¿áhœ|&¿å#ßYw¿ïÿÆߢèMAGNfsrqPKS 0315-282?ïã¤x""?\¡ÐT?5·Õˆ,—?0)¡?r­?i¤OË¥ž?ZæÓQ'è5?ïÐÊÜh†?wÁtwsÆv?E`>ý4¢ƒ?Nû°3:Ê>?tîŠûJæ?u3òp¦?ïUããÙr'?ƒ Ó¹íÎW?fásÙ.ő?oQlyèÞ­?'gUÜa)? '­›ƒ?ïχ3)fð?Vzò¡f?5ÄCÿτp?âæRÛP?và"#EF]?V'CË7ʒ?ï»Ýom‡S?v<'#ª?C¶bøŽQc?8ø[-{,?š{è=÷s?u^êϟÈ?ï'Æí èÿ?vÃM>™?Rܦ%xº?`ܚb¨Ôè?Œò¯Ír?‹ƒÚ¾Ñ,?îÏ,'{D?Gf"^œ?s¬²–ŽÎð?w'2súÔ? ™FìÜ3]?‹Ì "	ß?ïn(>ãjž?wb¸È3ä?GLülJ?:ͤêÎ?'€:¨Ê?w7Ú®Ø=AGN4FGL J0317.8-4414¿¥Ò¯6<gÀL´ûß	À;¡óQ›ÔÀ<ïq"§š@!wi¹'G?ýnvÖ 2¥?È0î	ˆiñ¿Ž/¹gP'?Ç?·e‡nI?ý\?r±£?ïø"à4ê¿à L jÓ¿ç3f"‰`¿Í›ÅÃď¿æ¢BŠ"?УßBÆ#AGNbcuPKS 0316-444?ï¬s~°gÅ?¡«¶?¿?4·?èÔ?.W'ص¿?"=gÓoœz?¡ªi.C"'?ï©êzG"?ƒ·p†.9›?Zm|éE?b+áLeÓ?'7½yÒ7È?€‹
~‡‰;?ï 1ñ"­L?‰sMdÍ?aÁžùÞ[s?`µ€ˆÄ¸?™Áñž'?ˆûÎ/1øŸ?ï:Ê:îŠÚ?~á'#*0é?aÔЪd†?K¬è⸥ö?–l‡
½ø?~iLå(ë´?ïŽ]¯øD?˜c©¿¡×?=†Í9»¶?1¤ÅN¯?‹|]‰ùŸ?QQ3n?ï?Eߐ?–>£¡&Î?eé†Ð>öN?r¶à=Î/ä?•ZA²D9?"ÔZ'#þ"?î|i2´q?"HÏâîý?e{•_;¼|?fP#¦DÅ#?¦á³†!9-?"¯ë¯U?íJ;vÅü?œ»V
Þ?|ÌlŽjg?p)l2GÃÁ?³âGZÍú÷?0ÒF8'{AGN4FGL J0318.7+2135?ënZ‡q41À=¢Ž£œQÛÀ9{¤ÆôFÀ<˳È	@ÐõØ´·'?ÿõ±]½Õ?´¨ÜW¯>q?°¥¿AÉÎì?û‹ÐÚè@	T¯ƒeД¿Ùs†Ž$¿Ùv€d¿â_Ïoº¿Ø|10É¿åE!ýÖ¯û¿ß
Ë |âªAGNbll3FGL J0318.7+2134MG3 J031849+2135?ïîā­GT?ZI‹?ˆß?2-m¨þ?+¸Œ?]ðqkIôo?Wix(U•¦?ïܖ;ô«l?p§«Co?AK»÷6ð?KßmyV?oÕv4$?l†-Þäí?ï¨p:êP…?y–vx|?SúÄ»[û?SÓõü*?ƒd˜½DÿA?Ca(aç‡?ïwöw§<¬?d;ýY¦?e^ø5?CZØüQC?Œª¤¯×?bmƍ³©[?ï㰐ÎfL?_ë$ñ$¡?AÊ!ÚÂ[?2d±,¸A?gÜæ³óHø?\ªS}Ž÷®?ïÑðçÍô?Š.Øõ=ô?Q©×dã?[ò{ÌëK?hàQ)Œm?ˆe|S+U?ï‹Ëeµ€?€Pî,]t?[v¥§Ý'·?PçP*`Ü?‰žc±>÷™?€}ž¨Z?îÀÏ>¨B?9™×"?y‰†ŸÁyÑ?aD^ù
‰2? ÁÛDCWÂ?™â¤ÛAGN4FGL J0319.4-7045?³jÛ¾r»
ÀDÕa^¿¨øÀ;TÔ«¾_LÀ<㤢â¸@ ÐtcT8<?úW£öíô?ÏûÉ,9?ĺH¦7Û?÷Yn€ç-?ükà£Ä¿ççΰқC?âÞ¨—c^t¿Ô›½ ´ëۿ܌"aFA¿Îº…@q4¿épTü±–æAGNbcuMRSS 054-102986?ï¿Haºýd?u›´ÍÊ?EڝE?Cý	Ä?}¸s½$­Æ?sÆ+¨R±?ï´Ä¥-mï?z?Nló?R%+ëŽ?VØÌy†¥?€Š1_ßÊ?v[Fø"b?ï`'e¨.?~Qo×e?apDŠ@Y»?[étæíñ?'Í
³'æß?|$W3Ö¹»?ï<Ÿ¨ô£?qÊ͚)?aiֿۚš?Jj]¡
¤?–QБ¯=»?qQ KRx?ï{ª–2?—pZ=˜?UñvÇQù ?EèV¸Ž?ŽWJ"<?~ l:ö?ï'Æ/F6?"±þÑgøH?dHdŽi?sصQ?˜u1ӝð?'±3‹•u?îã9šl}?ŠU·…«©?dø"j}í*?aAu~|£? |äΓyÚ?‰}HÐL‹?îäN¸c£?‹%všÁ?m{ܑQ¨?a@½¢?¬™ýK'˜6?ŠÁìï¸ý;AGN4FGL J0319.8+4130?ï@ÌÁd8åÀ*" _ñØÀ5Ó²Jj‡À:H¡¸é@oÊ·sÊ'@_&DÉ^?"sÚ Ó}I?°œ}#Â'@'<-ðÔ@ ÷½1ø¿Ç>¢Q#¿ÚáÚ»wåÀ¿â#%¿,P@¿áe°ÿì·¿å`ð
j¿æE~ßÙïËAGNRDG3FGL J0319.8+4130NGC 1275?ìþÜr˜_?Ài/ÌÿÖ?QG£jñ@?Ẋ
?·ÃýÝR?À­Ûß©?ïjnøþ{h?§–ePF³?oû).]¬?'}
Ռˆ?ewdKÀ.?£D8ƒÉ"?è‰Ê$W?³ÄíÐ'é?ž8M€9ÁÛ?š«Þ¯g%?Êͽ"©?³´"­âË?ï‹þ-x`?{~Ֆ™>?Y*ºóïA?SñÝ!^—Œ?‰ÛWÇÜ?x­ÍtÐG?é–iíj¸A?¾Ò‰Ônp?gÉCq—"?h*•H/ÓZ?ÉG3<º½Î?¾" 2Oˆ?îÞy"‰Ju?±¹µqP3?ƒ46qßU?¡áÊs¡ÐY?š–Àrâ¥Æ?¯@†"±j?énô悒?²—™AT?—l$p–£Â?—Š÷æ+5?Èà¿ 
ï??±ÉÃQ$À?î÷&#o	½?"¢A~J)?iêðÖæn?g‹/mÐ ?Ýã純?'±º郻AGN4FGL J0319.8+1845¿ÇV—%öߛÀ?²Ë…¤ðÀ9ârkWfïÀ<
øGv@!xH¥á%Ÿ?ùބ 
Q!?´½cù#ÂÓ?«³4uR't?øšc
»@;˜Í@åù¿ïöÇ¡Р¿–<¶áöL?ïÿÂWþė¿Û¢hu4¿Òܞ¼n/Þ¿Óg/x°kAGNbll3FGL J0319.8+18471E 0317.0+1835?íŠÔ¬Œ‡Û?ÊÅ&	F?k9½õD>a?ˆïÍr"?²ÏŒ¬·ˆ·?ɱpõOf´?ïè·T??iûͯ¸wP?,_•òæß?;X-åû?f82¢oÑ&?hìÒB®Ù?îyBOõ{? áÕÐ/"?V&󄟟?d±û|Çx?­×;Žía? °Ê–DX'?ï3X`Øø?n­êšü7Ï?1z6N†ûÑ?!oU­vB?‹§X(sN?nt Q§G?î¥ñEŸhÞ?¼üæ'h?hS'ðËÂ?'¢¦{Þ×i?¤³yd{ó?ºÔƖQæ?ﮏUP?†ïMÔiç4?>¸$ð'¥?R9\ØG#0?ƒfi'¢(?†$ØNNÉ?íð"Ps?¦Ø
x²šý?Z–.9«Á?dR÷J,$?¶®&¡šèü?¦Ø*à¯,?ï<òF%v?ƒ´
ú)>?=U½]ú9?97c?œƒ
 ƒkû?ƒ¨Ö¨g™AGN4FGL J0319.9-3821¿ìtóËû<ÀLˆ¦ YŸÀ:×ÜhKBôÀ<¤vtÑc5@JëêI_o@šތò?Ã0èU>v?¡"!ý=$?Ú'Òûº÷@	EBҍ?ïç/ï±Ô#¿â'eÀ¤"¿èÙà[DŸ¿é‹¾dª$¿Æ{ò>ÌC¿ïÿÿ" 5•AGNbcuNVSS J031957-381527?ïêÁ©ÐjÞ?açýÕ®GÑ?:"ìPºy?A¤P"i?aùøßç:?_TdòúZ?ï؋Š]Ü?rìe?´Ë?AOsؓàÈ?MJ«ðR4?qLps?pÆË´$††?ïiIù¯j"?"WLCÚ³0?ZgùÝ%ÞU?]'â	€J~?'0A4mÜ?ƒksrÏt?ïèö…q³:?G‰ø\œAˆ?'½KsãïC?MtÆrN?e¦= «?FÔ³1À?ïÐ3‹6™3?u>qÓ ‡:?N¶!bÎ¥¡?K¹°sD¥U?tv=:\?sª¯#k*v?ïœr}‡%Š?‡_ø`þ?JˆÔ"ûv,?UÿÆR>ü?‡:Óe˜5@?…û¯"Ù¹?îáÐviW¡?'?ÙË+‰?h¢N9?mœ+Ìaïë? XЅüÊ:?'sÍP2?ï²í9÷?iFw\O°›?CºfR£F?8>׌ª§8?'uËW°'?h–m …†¾AGN4FGL J0320.6+1125?À¢âØý²žÀB¤WÙÜÀ:·ŒR‰9ÐÀ<õ0™%@ Wò ò@… æ"ôï?Âó"`›2¿¥>" šœ?âhâý¹÷@2®Å$⸿Áe¶}ªû—?ì=ÙI²Ñy¿åç-É¿â(<县ⴜ>ån¿ÑXü…÷ü%AGNbcu1RXS J032037.9+112503?ï_…¿¶Ô?‰ö1éê¼b?[W è ?Nß­öºú?'iÝp1a?ˆðýÄìw›?ïžÍ'»…Ó?|†Í»Ì.?WXSMaâ?VÍy8Ñu?…ZË-(?ywœ<3Ôm?îm‰Ágò`?˜ªöÈ¥Ÿ?s´¢JÄ?o7KíÓ{g?¦Å-eü¤¥?—‰Þ2TA?íϞ3g£?‡J˜ª†Pç?tŽuO9?ZsµLZ#?°:.`¹ÉÓ?‡fúʆØ?îâF+æì;?•!¦Rk†?pSêÉD%?b7"'Ó?Ÿ¶ådô•?"ðޓ¸rç?ïÙü"Âs?""F4èv?edû®<ãé?qµñ_Ç?œx þ\$?']їaÛè?ìE2:{Ú?§…£$÷u?½‹¾ž?vc`âuI?»µ·m¦1ê?¦ðÁéVá²?ê
ºÃa6?¡ÈãAÚö?‹3Èb˜?yËVMê?Æ!Úûä'f?¡ÒãˆÃ6
AGN4FGL J0321.3+0425¿¿š`WÈW·ÀDÿ†ã´oßÀ:§S³ÜÀ</ý ª/@,ÂìÏ º@!_Ìr?Á4ˆó¯¿ª3j¾9?ê‹ÀBzÎÓ@äÉ?ìºåC¼s¿ç±à¸<¿æÏu¹Nk¿á|øCsW¿é&È÷U6"¿Î÷_]ÂíAGNbcuNVSS J032130+042628?ﱟ@2Ü1?x‡°?Y-fž)?J¦Ùüp"@?€rYxûí?w=¨ŽsZŸ?ï§Ò^~‡è?|²U4]R]?XÖÎ<ëA"?Z"£M~Ô?'ðŽ‡êˆ?xtð'Ôà	?ïQ€HBm?'m·H˜(?j<vR퍸?h6¡œYQÕ?'•á(N}¼?€…Ö¨Ÿš/?ïQóµ2Z?m 6	>?_ó~5'¼"?A¤d3ÑèI?"Âf Ù.ÿ?k²"u­x?ï
ÄKžäÝ?'óÊ»Æ,Y?sÐ`®Ø!?hjÃ+Z'?™'ÂxÇ"O?'¨Wp=…?ï"àY
w?"¨¶Iƒ•?dwÏ*¦A?mZ±Æ›ä,?™êK(l?'µ_STŸ?îdŸ7üä?–D8FËõ?}&ÅÚ-?v­–ÕÌ?¦:ëÝ_÷?"uwrW?íÐÐýÞèƒ?¯‰þ˜/?ztˆ0Ç8Z?ed¬1¶®?¯¤_ÖÅ?ŒW^"=—ÄAGN4FGL J0321.3-1612¿ãë–Ñ_¥úÀJÕf@¦¹=À;p%FáeáÀ<Ä#G,å;@/ëîÑ?ý橝ÛÙ?ܪ'zÁg>?ÔֆŸkë‹?ýÕ½6VÔ"?úBöt»ê?ëw¥ˆ»%?ï°iŠU_¿áj¿ÜÌú61ë¿ä,HÐ(¿ïù"O¶!AGNbllPMN J0321-1612?ï±ÕÁyBÈ?t^ϓ›W?QšÅä›?Dµà‹¯Å?WOSAžð?s2†"–?ï0Á»™2?¡c2Ñ?wª,"ðˆO?'†"
,ù‡?"ý=†\ö²?œÅ,­M¥?ï` ÿ"u?‹ÙtqšE?w€'¹ê¶?w/-˜Ö,r?–"Ço+6.?ˆ[%ÊÒ½?íˆ'Õç?TŸ©#†?ŽZáñù·N?z ˆßU?¯èÎb³…Q?‹»Ø3¿<?ï'ÎK§ô%?€ÄŸü¡?aôIíw¥É?T0£ü<½?ŠÏZ"éC?ÅÕB'R ?îL€7â‰;?¦Q‹×ÇÏ"?"ÑpˆnÈ?‹£Sæ1Ì?¦ [p7L?¢ïÎWÐ?î±~'Ö¼B?"4OÙUH?~6ux??|ÃÊAò†¢?¡!NÖ¾q?{´¯´3?긻Axßÿ?¥	˜j{'?'',J†¿?‹y‰ü'?ÂØ-fs/*?£Ñ rÞÔAGN4FGL J0322.0+2335?ÒöÄK¸©ïÀ;˜§'h˜À8ßaúÆÛÀ;М·[K€@^æÀ=ó?ÿƒëaãIç?§uëƒ`?‹~Ö¨KkÂ?ãYA¥Ã@øù²%?ïô5â:\¿àñ¦ é4¿âúúÁ»¿Û'ýûÉ¿àÃhjL¤ô¿Ùº å¾5ZAGNbll3FGL J0322.0+2335MG3 J032201+2336?ï¬t™K}?xú?-඀?P¥Ÿ×ŒF‡?C+—Ì"¢~?'Î%¶Ìœ?ws1\º²@?ïÑð'q(¯?t‰šBìÍ?GëD¦?S	Ѳ°Y?t
DÖärÅ?qTµ`Šßa?ï烳6?'=¨apxÝ?tý襧¹'?XfŒ'ŸU?—C•sG´ð?wþ",•?ï$èNªÕN?u¹€Gk­?rƒpœ""?SX(ÒÐQ?–Â(¢¥?sc)"®‡?ïMgèØ­<?²Ý²gÃ?dd݈/ß?\;û©#ý?"Æ€ÅqÀ‹?‹`~ߝΡ?ï}$ Ҕ?–B)39š?S4ç³ðí?cwYíy?ŽGc4Ë?•;¡Ñ'x¶?îkAƒV…?˜=ï u¨?|p½"!øT?J£'6s?¥½Ð(Ί¥?–eGò Þ?îO?¥©À?'
<ñ'K»?…æ&´ Ò?oKä®åŒ?©q'X@'?Žĉÿ•AGN4FGL J0322.4+6606?æ<rՓ#@Teè'%1À:%½›¡æÀ;¥KJ-'@Ri|ñBM@TÓ¥¸?Í%ÑuÓì§?Â(ÅÆôÄ?÷¡w´l"@mËÑ¥#»?ïƒß=g¿'¿ÌŠ|ºe¿ç
@/p¿ê¬t½—$ʿ竊\å´$¿ïòªa½à AGNbcuLQAC 050+066?ï¢!Ø-Ë?{*íäÔfX??‡{yá:?4xñ'X±h?†{'rڔÁ?z̜±•#"?í<~™õZ?°œƒùõ$?qÇè•_ã?yTvhSÞÊ?µ
Þ°mÿ4?¯ÆnV"`"?í4î¢h'å? "f˜ž›?ˆ=á?º=?†~»óß?³PÎÍ`¤
?ž³Utª?î¾Ã7€R~?{¬ÒÉp·?n¬¹º_ó?PSï¡Ûà­?¢)ùPî˜?zMÙ*"ÛD?ï(1
u5?.²êùø?MB½ÓBÊ©?C™=¤ë*?šȽ!Ö?ÿe1Î}?éëä·q"?ÄùdQیP?ƒž¶›Qd€?"±ñëon0?Êre
Km?Ä j‡÷õ^?êߜuBo?¨a眆ß?—¯"cÁôÁ?'¾4ÿG;?Á‹o3‹ë?¦•¿I jÁ?ì"Õuùèu?˜âżÐ:?Ñ´rÍÏÅ?lV>U?¹'Á«`?—ü¶•
AGN4FGL J0322.6-3712e?ÅùGÿóìÀLX±mÀ9ÍàöO}À<Oʪ³Q@ÇìÀ24±@9‹q¸ª?²ðìçŸ?¨)>'·Ó?ö U?Íui@¨ÕzÆDÈ?ïZeÁû¸s¿´åcË+¿â³KQ7*9¿âÇÿÞr¿¿á>ÀÚü¿ÝŸœèÙrÍAGNRDG3FGL J0322.5-3721Fornax A?ïÃå‰¦2?hǣƂ֖?I#ÏôÖ
?7µ˜ ج?zÙÕ\‡ý$?g_?@ÎQ?ïÕ©Àª€?rf‡É
"?E·d Üœ?Nôî(?؜?rtS"ÂÁc?oyi1I´Œ?ïS­fe?…h8"ž
[?gy'Nǐ?eqGBÔ?'›9®Æ?"#µåF?¦?ïhÊÙ~z?gÉZÛMƒ?môúbçÕ?MúŒ÷)R?ŽPN÷2?e\,Iá«?ïf~ƒàí
?ƒ¨—X¾9?aædɑX?O'1fLz?'r´‰|D?'x.?ïxªC¾yV?ã?ÿ*?\öƒ¾ÄË?e¿+ð‰?Ž6žp…ý?˜A°'?î]9­æ?˜ÑçIíã2?z-í ð6?y‡pD?–?¦á>¼áL?–ÎB#Ù&Œ?î˜Í\G\>?'ê¿îÄK¥?§ »rl?húƒü
Öý?¢	B
µƒ?€i‡AGN4FGL J0322.9+0940¿î@g'û	ÀCŠ'¥aNÀ:ËW´ûßÀ<$ý~E€=@òÁ	J+@1fàé´?ƑཚÉ¿_Œ‹Û?¸*žd.©?ÿ›£4"¿î
ÍHÏD?ÌfH'ZŽ¿æs½œ®!¿äYQªí¿á.¯½µƒ¿áìà¾q?]AGNbcuMG1 J032256+0941?ïoäA2¥D?"S=º¸Ö?Rޔ´þ0?D}|çâ…?ãð`¤?ƒ«™'¯œ?ï"Ô·c^?‡ÏȶzN?[{<jI3ø?a"s¡ã<?‡›j‹+p0?"þG…ÚÞ?îÚÇ,µü¸?ã܈׃?r.U<˜BÊ?o½€":	? 
Œ1E*?Àð2ž?îfÌl›Ç?€šÅI½ç–?e«ÒO"?LJn¡Ab?¨8_r ?€LR&[?îÇhß½jY?•›ÃÊ­~L?eÝå.³"¶?[ñÖ° }?¢+"­v6?"ƾ™B·?îåE»ºÅ}?›ØíáR<y?fx¤ç3‹?pPÜLUÈÑ? D÷'?ü?™ýÛÆ6q?í_Tª.ð·?¡}Y¿[l…?>÷ÕZ)?y6Oq©!ä?²ÝˆñP›Á? §ÄË8²€?ëréî)?™Õ#đ{#?{yc˜IÆ?kiæ³Ì3?ÁX\Ô.?™'¤–InAGN4FGL J0323.7-0111¿Ï»؃hÀFœÙ¾L×IÀ9y|"MÀÀ<ýð[GN@²S~'<?üöñý2Æ?³†þ6|>?¹ œ,ÆÝu@ª`%څ@ã‰û÷Þ?ïÿ-<y-¿ÅƒÙ¾Í±¿ßúTvyÚ¿ÑyzϪ¿å†Ö]ð 9¿Õ•:¤Á•âAGNbll3FGL J0323.6-01091RXS J032342.6-011131?ヲÍsÎ?pB¬³¶Ö?B—J²+ùw?6Ï["ÚZ?~Ù°Ö4ñ?n‡þ2h¼'?ï"†RÍ?šCX)d?{©î±½š?†`EÇ·?"Đ~ò?õvÒ(Þ?ïŒ-¡¬?"¶Zðf…?sy$¯cç¥?pÖTëô–?šÐ3òf]"?Š´!Æ~s?í=h¨év?ƒÂz~˜V¹?'l'T¤èš?mé2|µ£?±xÐc׬)?'."š0Ø7?ïdÚ¡$ö?†ê
¡B?\ø©Hˆ	ò?R½€¢?'•3""0°?…µ©#T?íÇ$‹`Ø?©½=9Ã?Ž'ªš¦g'?–>ï:F3&?«êX&›?¢åÆ$mÝ?íÉ;Ϩ¹?œ×TTüÿ?…‹¿nóÜ9?€¹èàNî?®	S&GÜE?™"qFò¶I?éÖz]ò­?ždþƒê_ú?¤J'ÂlM?‰oòk?ÓqàÃr?›²†ÿ‹AGN4FGL J0324.3-1313¿¹ŸÝ€y7$ÀIÙÕ<ÝÖàÀ:ƳÑSDKÀ<rºÇË)@¾Z.t²"@l'	Z?ÅÔú˜¸?¥CÃW®?àLS?È@f¢$'–H¿Ñ-!¡:wË¿æ<¿ß®Q¿ç/SàQäÏ¿ã§CÁð`¿êÖ
ˆ~¿#¿ïþašNË?AGNbcu3FGL J0324.5-1315NVSS J032430-131002?ïÂWš_	?nnõûs&?WúÃHsE?QMêd?xՁé…s?jv£ÐË#E?ï¾/5?y³Õ¹ì/?O‰ºÇ?X}#?•Ú,?|ð+ã9öô?ua˜Ä°Q?ïró'n.Ý?~£{.o`'?j'Ȥ§õ<?p^ØL
±?Œž­2[O?vÓnË_›?ﮃ
¶è4?]%—Aº/?U¯ÎÚî°?7¶¦ub»?©C¢Û,?[{l5¡?ïZ^'tí?‰+&ñdz&?m=Ÿ@¢/‰?dË:ù=ª™?' Lš[?‡N+KK?ïC-^KÕ?—x84Ÿ¥ê?_¤,ÁÙÇ?m†/k¿Ìø?•£ÙëÛ?•±êë"-ç?ïaÁA‡?†7Ü"EÉ:?q@cÔì?k=ÊTG½?™ƒÅ-,o0?"àl«ë§?ï*-%',?|ê=óÃî?n9€Y©ç?WOGó(?˜³ŠVf±=?zqGöx¿AGN4FGL J0324.8+3412?Ì7ôß¡¡âÀ2¶®::ŽqÀ8­<Íè«À;±5WСn@—#ȇ@)@k*?¥ ‰ª
Z?­‡½Úy?ÿÉóÔx"@#ò‹ù
¿Ù뎃æÔá¿çöÌ ,/߿ꉢ«'â¿éSÐ↏¿îcó¯5?äÆ@–žAGNnlsy13FGL J0325.2+34101H 0323+342?ïø'ãÇæ?R?úI8To?/;á5
n?KX¸Ž>@?EÍ!¦àA?B*ï}z?ïìúÝ\?gw\w4ó?1ø#S…€?BÖzêA…™?`Æî–=?dµªYúÚ?îÞG·µÊŽ?˜ßd•[?ù¹è`%€?‡…|?›:,.A~?"AhiƤ1?ïôÖèÉFt?=v&{ä›?3V9©Wh?ÿ•Ä­í?Q'YfF-¨?9é&Ѓ*?ïô»zƒÃˆ?QtM3T`=?2ÊÒÈSd?-й¤EÏ ?QÖVqÒYl?P ñ)(0¯?ïÈÔ
øó?)V½?Fȳ	àøn?XÇWàÄ'ñ?x¼â»ÍÔ:?ô?CÜ?î[ô
\?ž¶K«úð!?€eÚxÿ"¤?ƒ»Uƒ ¥¢?¦'H¿ó†±?œ+ôÖá?ïÛ¼)oÃ?bL°´\?S»`yù|?H
‡É½QU?j½x¾O'þ?^Ù±ÏRÞAGN4FGL J0324.8-2043¿ë™ó±	š*ÀK?™ÜµxÀ;hi²KAGÀ<ÈõZŠ@ "¤Ht8?鏂¿b€ÿ?ß>P}pï?îøÒpXƒ@i΀+3Š@	î…äÛâ>?ïùÈþáòÏ¿ïñ"ݝ)œ?ëÈòíÈÅ×?µnTœdz(¿åvpnö¿ïÿÿ" 5•AGNbcuNVSS J032451-204324?ï3A¿y8a?¼Lb[æ?dEìý#—?½þ&+ÐÎ?—?PyŸf?¹¶ˆ½©C[?ïžýkóÞ?—‡£U®²?`Ñi†Ìû?w8 µ¬	?"w¾š³_?"Å"d,y?ís´0"éE?¤WÓž×?'B›DbZ;?…='R¼K±?²xe"?£­. ºs?î¾¾ˆ«#Ÿ?'Yä?Kížðuš?@{\ÏA?£§ÃÀîùò?']ì~ʵ?îŠ=¹7Þ?¹U.+½3?xr(Ö&×t?'czl»g?¤P‡ò0?¶BlñÛ
?ï$ZÝ?£š}`_?tZîö.Ñ=?'õ	Áo­?–^§•©Í?šqŸcu*?ëÐêg¬%|?­²9*q'I?_'¢G?ƒ|_P5`)?¿'ºHÕu­?­U¶€Z-s?íÓ™MI?¥•?¸@%?GI(Ö÷?Iß·`êŽ)?±8pçå%5?¥¢Aè:ŽAGN4FGL J0325.0-2416¿ï›ð›½ÀK³w ÈÍdÀ;[s¶±•À<µ\ÿµ@ßý®ÁôØ@]SG¥°ÿ?ÂÔé¦Í3пµ×"z,?òã<æ:\@hNAy¿Ìb{ 4hg¿è÷ÿ¶.$Ö¿á•+uϏö¿ïì;ýÝ?퓟ïôð?Ì7
Þ:ŽAGNfsrqPKS 0323-244?ïåZ×U֐?ƒÍx"S?1@<ê??ö	f9GÓ?h"Hæ*V?ƒƒ;>[Ž©?ï°õM@òÜ?‹Ë‡ÅŠ!ý?Y-oš-?j?öE-:?€©Œ%Ä?†Öóùï?î>CDJ?œx#8V?h؜ò.Ó?sÿž´,?ªŽE½e
?›î´LOT?ïöšŸÓð?Ez?Ô>â"6.yê¨>è>õ*9°?SÁË'¸V?EWL–—±#?ï¬,¼ ­?'7'}‹u?E‹aÄî?I´V¢e??ƒœîdíV?¼´!©J?ï\ôƱ/?¢LºBÜs‰?\l¬Ö¬,k?q_¯vÓVŒ?'šœn£0M?¡lu´ó?í€$Al¡?¡õ1)t–Ë?tlçp§\?v_í–:þO?¶­5ý™Çˆ?¡¸d9TNP?ïÌÉßT]?pòóÛ5¡?2¦ªÇíg?râððZË?yb«O†Ž?pÛÈw5hAGN4FGL J0325.3+3332?åkÝðEÖÀ32|EÀ:ۘkœ0MÀ<(ŠÅÁ@@ÞÜØÞ}ú@Ñ1ìVu?ο'½†,?¾¡Åg}¾?ò¢}SõÌ@Êãés÷t¿ïð£5úÐ?ïýâƒî6ª¿ê¾ÝöÀ¼¿ÃË`æõ—ò¿æ£Ò½§•Ü¿ïÿ'ò¶kaAGNbll2MASX J03251760+3332435?ïs¶î¿ö?zœÔ6£€?Z¶‰ð~_±?Vè'ô¾"4?»sż¬?'©Z´Ñ?ïÄ(ûï¤?}®BÍÌÓ`?RŽ	D	@?dÏâ?H"í?yGÿāã?xjÛx†®k?ît'J€«?—ýNÇN¹?{V¥L76?}×¹e•ô²?¥M»Rsb?•ÒVB™&?)ÃY?‹gZÚ~?|áñÊL²¾?bZwáj–?¢º/+à°9?€rÛ¥'Ï=?îÂeòÀ?š™^PçOå?|øªº?{B@œÉ>? : œº'À?—ïÊgg¤F?ïM0îÖ?",I³H‰?h´ C‹Æ?uN	72'?"CkÃ%6Ï?'ˆ² (Ì?ìšÝ8°?¦zÔÌ9mÏ?ŒI7( µ¡?‰[hQ:>Ç?·ŸðúP?¤£—K!?ìdØp*Eµ?›$""95ë?'(l\~îä?t¸þR›?¸O!g # ?™¬ˆ5xoÄAGN4FGL J0325.5-5635?é†ÃѺÀHé*0U2aÀ9ÞT8fxÛÀ<c!¸·l@¤&ó?þä¡Õ¨>?²@ÊžUì?£Sþk«?òTE·š5¡@´2vÐ?ïÿ˜ È¢q¿ß°Å/Iš¿ÜÚ\FQô¿á3ËÿY˜¿ÙÏ:û©"¿Ü£¸AGNbll3FGL J0325.2-56341RXS J032521.8-563543?ïôÊØ*ùÔ?D5©·Ö¿?űQÝOQ?	¹›4µÝ?TÝôàb»í?C"L«šµ€?ïë.±2+e?h«ÆÜ4¬*?+Ã.ÖÑ?;Zà%Ÿ©g?c¬/̶?ffR߾Ɂ?ï›òC¡6é?|‹ˆ"ªft?S«õìr°Õ?V¸	PF£'?†ð`S;Œ?|€¾<¢Y?ïÛ×[
¤?LS¸ëºã?<æ*MË?!jqvråù?pEïÏavÅ?K6Ö+j'?ïéoÔ4†V?Z
?³fÍ?/™+ĝ?$·¾lÇdD?džAµ@Æ?X•w žd:?ï¼#œ½:‰?'…ƒíŸÓ?;Ò¢÷Å?N><'_´ˆ?€ƒ§èXn?Dˆ%–þ
?ïeZ)cž?"Ô-ã>Þu?]ÆXÚ+Ãõ?bBN€º?'xU>Z_›?"?NC·¿9?獵îa?i»Êñ&ZŸ?PüT '
±?=>Ï<ĜÂ?"6yí4~ë?hœ™U}ßAGN4FGL J0325.6-1646¿èøáZð´ÀJwÃ?…Q
À9'BG£-À;æ³ «Ü'@¡ØR¼æP?üÖ#l?¬bjBD¸?ª—ÁA;J@ìsƒ…[@
sd{ª›¿ç=†É2¿Ôëˆy¶¥C¿à-qÊÛ[¿ÔOóÞ3§w¿âEœÂC¿Ñ,`Eºõ4AGNbll3FGL J0325.6-1648RBS 0421?ïõ\¶9bw?K¨pû1@G? š®ßdN?S'; œ?S3==NõC?IÝôjŒˆ?ï䠁y+?l‹&ÃÇî&?7G'é† ?D8Œ~Hi?hwc<´?hÖ6¸4W?ïž÷/!?§ñ?Ú Ê?W«ú.VÂì?_`PNÙKE?…‡'ðÔ¡ª?~}©³Ëÿ‡?ï~'BÿÉ?j¾é_h?Oöc¸ô
q?3ù'&Hü{?Ž`û½€H?iѶ€–?ïáÑXî?%‡0mß?@5Ë«3i7?Z'\.?j!~ïåü­?yƒò3}Í?ï²ZgÆ?ƒ(Ð㘥X?FQ‹ºLÂå?V¨·x¸‡ ?'M~ÐJõ?¾ZŠÄ£?ïfÙXÔàö?ŠÁÀJãr?[XLJmü?RÚ¨?•?'s_Yhj?ŠP
'wÉ?îÑÌI€bÍ?"JýbÂq?b¶Rë¿ì?PtR(<\?¡·Ö7q?ƒ›§QšQÒAGN4FGL J0325.7+2225?îkÆ£ªYÀ;ù@»±òVÀ8¢ÆÅKÏÀ;Ä"Ÿg8ô@G¶h‡Rð@K%}h
«?¨íöëÁÉ?ÅdI,@öøj	‰@²ÑÖKý¿Ø1—׿¿äª¿_»ý¿èwÓ«äù¿ë,L$Ì¿íîa«ì¿ïÿíöé	AGNfsrq3FGL J0325.5+2223TXS 0322+222?ï½,[Ü'f?xûâæF÷Ý?u5pÜ(bß?r‡hGDÀ­?hh›¢[«?e,æÐ?ï­ãv.z?†½/‰hF?_‹%õ÷UD?p"Žâé¿+?€•½Ãü¸Þ?'¾·5éê?ï/Sœ#%Ž?•6ÍPé)?ˆ[ͯk€?ñá·É
-?‹ÏKU‰Œk?Œ€ÔÅ¢]¤?ï°Ï¥¼Š?cå—2ÄË?pÒ!A?Wœ˜¡M?w–Zþ[îœ?Yiýæpoþ?ïŒä¤|C?"}w«Ü\û?·z,¥P5?}iD?\¥µ?v¹~'U}?v4»¬:œc?ïÍ¢›Üü?¡j<¢²Aè?zéÌFÈò?Ð¿Æ`i?˜bQ@Õ×9?›¡æ/¤|Y?îúÓĞç?–¾ŽÛ~?ã~R?÷ž'ãÞ/?'"©Š}r?‹Ù¡·ïFÕ?ï#&s\æ?'ž*ÿÑ?‡bdB,œ×?tlbÜõ‹?Óþî}¹¤?xýf>kª,AGN4FGL J0325.9-1843?ê'ñ¹|tÀJ̹#¢œxÀ;³"â{À<‡¡†`@aA¹^@£BàO`?ʕΈ䕖?ü–"¨q?×jîöÃ@\@c±^²<ÿ¿å‰ÿ]BÑ6?ïÁÿáø¿é. À4
¿ÕHãß
>¿è^ëÈRj¿ÔX£š¤["AGNbcu3FGL J0326.0-1842PMN J0325-1843?ïÑN
o´?g[üfS­7?>­cA@+²?4Ö@-¿K"?un'1™5?fWµ\ü¯?ïáv}"\F?kÁ8!C?5›©ûT?AŸºÌkgP?kÖ
*{&?hۄNÇvì?ïc‹Nõ~?'Úr~*?_cd5'‹?Tœ1–›?'§T¬÷è?'0ùwC¼?ï±`4É
?Y8?P.òhÌ?4ïCø¨?z›Ë†|_?X¦7Òt@?ï–P´xm$?}~`j½Oå?WŃXÂÀV?e0‹è·R?‡s"o=:ù?zX+%û?ï©Ðã ºú?…m=JWIå?H0}ñ		&?Xµ'¹œY?"¿Z¶o?ƒ‰ãx*Î?îþiöÏæÄ?ŠõrãkWŽ?gšt(OŽ5?cûš[ޒ??r¥œ®¸?‰2etœ?ï`zï_sÙ?w­ÈÍÔ'?cÓ[?Rtó1ËO?'~‡¨'l?v7·Âȓ·AGN4FGL J0326.2+0225?½¢™×ÀE5¬îàóËÀ9RÁmóùÀ;ý'€ ¤P@ )j \×F?ý™SÃÌs?²ƒÆôp«?"¡q\í?îFTþ_@:;j?ù?êEXßÀ‹¿áp^¢LƂ¿âsEaÞí6¿Ô£,å¾`¿×²!vrM¿ãûbâMhAGNbll3FGL J0326.2+02251H 0323+022?ïÚU$Zäc?cvµÝ%Ä8?9²uñR½Q?,Q†¥·Y?q:F‡¬¼Ì?bKb¸ßc?ïÙ´]®ö'?p{þ±©äH?=…{ŠÓî«?E¾·ÎY¯?qMyQòÞQ?m8Ëې?ï…ÀŸJ'&?'¤ðVÁ
?[\EÃ\`?\£z•à¸û?‹$Oj¡^Š?—â÷9ê?ï<oÛ7Ò2?oÚy èÚ?]£œ$×Üf?>RqûCE?–—ÊØú?mñ('õM?ï›õú÷
A?'¾Q¥]Hæ?SàYa?G)M°§È?† AI8'Ÿ?îsPZ¼‰?'ªü‡?ˆxðk]R3?I)åD{y°?U5³¤0n+?‹F½=]š?‡KC:áT#?ïŸqÓ_—?êáÃ{€¯?g[zxêì?nøGëJ=?œ@±¾,	Ä?Ž+²æe²ß?î'ŠÃ'çN?‰/JíÐW»?r]öÂ?\€'|?«;³Æ|·È?ˆ,ú4$†AGN4FGL J0326.7-3404¿×0òš¢êÀL	U`"¥À:ÖõtŒÀ<Æ$)ªô5@^ê˜Õ?þb,•Š@`?Æ(¿ý0—Í?É(Äûb7@C]œ"I@éj£·Õš?àMÍþ¦
Æ?â$EÅ.…±‡!¿ÞÉÖço¿ìÏ‹¿¼¿­"ŸÚsAGNbcuNVSS J032644-340330?ï¬óÀ£ëú?sFíÁ	XB?fêhD7W?\¢SCuRï?~ëoÛM?m«+mé%í?ïÀ]åRC‰?xµ4žŠI?S¢$»1°?Y–Flb·*?zè"FÌÇ1?t3–,j'Ï?ï(ÎÙul?ŽMêÕ²Š½?‡"'™+r?‡‰«ÙÅÖ$?ŽH"´:Z?'39"?ï‡#N¨sk?eMÖºCÙ?nn&	™z?R	6uâú?†›¦"Ñšï?a"‰c?ïk;ã0"?º*]ÑU?|¤¼ÑlŬ?rÓrNÃ.Ù?†Þ¨½/@?x'èñ?ï\—~{?'ÒaQÍ©Ì?_óüÕë¼Í?g«æQþ?'mÐX–›Ã?D,(Á¼?î·Ê1<
!?"b®P(ð?+èK ?íak ¿?šq6f(þ?‹…«W"Q?îë݇KÊ?€â³X"|?|5ÒqÑä?j‡‡ÄÀö?›vèI9?|?-ô¤<AGN4FGL J0327.5-1805?òÒߥÀJrGE8ïÀ9þ\XÆj³À<3ë‹Ô´ù@ñÓ"§IÛ@‹ÞZ"ÊM?·Ý­DÇ/T?¹@1¸#?õõƃÝp@Ä E°8m?§9ÓtÝ¿è	N}'{=¿ìòwéF¿ãˆ$&Oõâ¿ëñ–¼ˆÝ¿ïþùÀJÞKAGNbcuCRATES J032743.34-180342.0?ïõ'"ef?P9½4ȇÓ?@ªÉæ{?;Ò¡¯s?IäD wÙk?Gµ¾H´f?ïéâÖ¾,?o"ˆ½_»·?2Œ 8Þ?G҇`;x'?cË¥M^"ÿ?jزPÐ(?ïBvßLá?'Cÿ«é ?p¢lŽåÒ?{C:±9ší?"ˆˆû×ê?Lú:¶b½?ïò:ÎÄ/?;Üü§G…²?9Ç4|,¬?#À‹c'JÏ?U‹½>3ŸC?7÷öÌQ¦?ïð8£ÏA`?VTÊûm÷c?Q^=š?K`NÁ¸¡?LahšH†"?K¥+E'ò?ïÂÔ¡'q?'bƒ)ñ?BÐaØý¥?]k_þMu?|f	žã#1?€L˜&­^â?ïm]·§]?""Fñ?wˆ·9Æ?€ìû©¡©ÿ?—Lr#§Ý§?1o†(2?ïÕØ/	5'?_ә¡'?Xù0.Ñ7?KS¨Å¢'?mßT)J?Xàè"ÔºäAGN4FGL J0328.8-5715?ØÝ[p5rÀH‹¼¾aÐÀ;žJœ	¶À<ì^ª°BS@"t˃÷q?ñ×ôH;Ù?äoñ•1ä?á—Ïà'~@˜"?úJVËhɘ¿ïå¿Â£(9?ï–Á¥)ñ¿äÀ€æDm¿Å3ÃçJýT?¦à±[,K¿é}"€U$öAGNbllWISEA J032852.69-571605.5?ï°Z"tf"?z$ٷ?P'‰T/Â?E†r/È?×	ûx$3?y•ej?ïeÜäÙ?Š·©"nW?d4.I?qVº|?†Ù}#0œ?ƒªCG–Ú/?îà3ªã'?'"óê<?ušf©pò?xbØ,öYî?ž'ð÷¾+ä?Ž…rMØÙ~?îb¨õ¾CÙ?‹8¡ èÝ?\Ä͗Õv£?U"(g'ð?¨ïJ8þç6?Š¤ôâ,¿Ø?ïoÞÁŽ?†±ÅÁ]~?cóa²/¼(?\»ðÚÓÿ?¡òYN?…†(vS?îÝnú£cŒ?¤mÒ˧N?sáËâ%]?Šô[*IßÛ?ŸY­µI0? ÄÂê°>u?îO
Š¾E²?—8'OŽ?xÅþÁ'g?zÚ·éR¨?§ögxOÁ
?•ÌAÌ#Â?ìJúí
Á?¤¨ÏÝòeÃ?aOä—b­?qã
k[Ë/?½©o`Ç&?¤(BåéåsAGN4FGL J0330.6+4659¿Ã¹TæÐôÀ™tNƒÀ9•¶åû7À;ÀcK(ó>@<8?Œˆ@oÐ!ëã?¾ÿ·ZʦØ?Ä/â›Á-@Ɣ‰`[@g+Þ*B¿Í—£ö¿åz¡–'õ¿éÎÚÄT®¿éêÿR[§¿ïóȟ@¢‡¿å¶]õ~AGNbcuB3 0327+467A?î9Øe©Ÿn?Ÿ±s¬ªUo?…š•žáwÂ?'þÀ8R?¦ûÔ>‰'5?›~чÀªà?è¶:
§ú?ÃAƒÃn:?''{lG]?"3ðd¯í?ÊöÈq¦éí?Â9L¸ür?íoM œÃ?œ@öh*ø?'"µ7QG?‡`nÇâ@ø?°&Š¤Ñ^—?˜b™²©?íÂíO¤-?…JÈ  Ï?•¯"Ќ
j?st©WJ<V?©Áéü?€ˆBé{?ë\šu]?³þb=¨P?ž¸cµç@?–¿o}L˜?½mb?K€˜?±S>_q?áœ!÷ÕÑ?̟Ï9tÑõ?¦vc´…XD?°!Ñ@aài?Ùøï™Å'V?Ë|¡?é+!'C<?¯2éêÈhî?«QÂÇ8®à?}ÜþüU?Ä
Ó~Ó×?¨¼e¡o{ä?éÛ«ø@îÞ?¡"s=A?°Yþ¬¡fË?•e¡mÄÔ?ÀdPÈ«'$?˜ŽÊVßAGN4FGL J0330.6+0438¿ìÙGÿóë ÀDã>ÿPÀ9Ï"M1âÀ<%E«Hï@»ƒú @DÀßXÀ‹?º½<áÝ«?¿C¥`$Õ@»­À˜$@十×?ì۝_¡Ñ!¿´&,9™Ô¨¿æŸ³%]¿Úþ$þ½	á¿êý՞,¦Q¿ðAGNbcu3FGL J0330.6+0437GB6 J0330+0439?]ØUö?¼º?`î?pHT³$? äÇ}H?‡­þ3)֜?µdZÏW·9?ïؗ!ÞæÅ?u÷¤›d"?A퓑(£î?N; ,-½d?qv¼©êÈ?r"`"èÑw?ïp=L¼œ(?ˆl?]ƒ¬?w~®©ÇŸF?y<¤ä?ˆ1U†›ðI?y£üê6î?ï­ñ|¦ç?a4kÆ8eM?]§=Åõ?C9)Öõu—?€ÎÀ¬ÕÎæ?^-}Ÿ¼–?ï¤_yso ?­lå^"¦ò?r)÷IFö­?ŸÙEæp
J?{¦LÝñh?kÓç?ï"	cغ?ˆ©·È#‡Ô?LrLÛ{@?W•'¯74?‰6˜S¯¸?‡. šlaÚ?-÷Æ?ÃM †m¤?€dŒ3
ª?ƒöݨ£]ú?"ùȽÐXé?‰ômçPï?ï)-ØJî?~Z'Ÿuô?tH:˜¸Œ9?a'ZÜ'²?•È6U #?y››øÄ'AGN4FGL J0330.7-2408¿ë½š£7…±ÀK82vtÑÀ;b«ð´2¢À<Ù£€£(@ *Ï·bØ?úM "Ú?Ôä< DXŸ?Ïpk"ð(?ûãèrDÁ@ƒ¼|±¿ïʒ€Ê÷?îrE ¿×¡P&kú¿ÒtZÅÉM¿æzÐKŽ¿Õ>ê šªAGNbcuNVSS J033050-240612?ïޟ8¯—?tÝ09/(é??ZUõXÏ?AC  ›°š?mu}HÀº ?rê0L±Y?ï¸uŠÏ/?zß±t5jÉ?R5V†nùn?W±‡`¬Ê?7åIžÒ?w5ø×b?ïsBdËÔ?z‹²ä¸ã¡?eR§rýõ?_-ñýIF?çE˜c"?xË::-4?ïúÞzk£?u4az$#˜?j2ÏÙú?Pä­Ya¥?šz`gua?t
lc¿?ïÁG
•?n¢Ð1(À?P'²] p)?@óý)j>Y?{PoÜÂEX?lx ‡×?ï>çVjû?'S€¾R÷Ï?bÕÁ;ڎ?m¿9ŒÎü?•È]!A`?'*P£•ø¤?ï#dLõjê?"A*+r€˜?j´þ<ŒE?a"a¬ åò?˜<ò¦Z…"?ƒ[º=æÜ?íÖÿ"kEZ?ýŽ×5ëÑ?sWЌÏûŽ?h1Cb4?°†Ó3è<?s³ÃöÁ;AGN4FGL J0331.1-5243?áµ·š4äÀIsüC²Ý7À;&ê«Úä¾À<ÃNÂò®@H‡r¦@yýåsŒÀ?÷øX$Ú¿š÷•ì¼?Ô©S æêÛ@É(Åñç9¿ß˙‹í¿âþP",O¿¿é'A¦"} ¿àXÍ¡ˆü=¿ïÿý±q&´?äQªí~ôAGNbcuPGC 013066?ïíããJ?UcCÎaN†?EkÚ#OéM?@ÀFäk.?Y'Le$B8?Pgð€æWS?ïÎ d×ù"?uçÛæÚ
ì?G.í¡°]?QÕhùÒã?v	ïÏÿ"Í?r¤´º8Hç?ïНfا?~Á–ÆïÖ?eòúL
ê?hë>uY:?ŠQ[E?zºµÈ~l?ïìürÒ©?D…@÷5
û?8K'¾úö?"Ðqð®–B?_ô6Gã?B¢À{°ì?ïßf&
è?c=B>N?T<ƒ¤ç;?Ou"Ñàz?fÕXȜœ?_(qï¨?ïzÿ6pCN?Žå"®s&…?U!Œš7µ?d³å{j?ŽœǾ)£?Œ{«+™4:?ïÚb!À?‰ûµÁ?q¶ÿײ?tp݋Rƒ?™,þvú?‡Â-76?ïÁQ½s#Ê?fCÒñᥓ?T™ð	w?G'"mŒ´"?z0¥;Á?cþIz}¼AGN4FGL J0331.3-6156?ëÛÀ8GwÁÀG(µÃ›Ë£À9Yėt%À<Jè:@X+ü2@?ÿbBw†?®™½
ù#?°êÀŸÃ@¥:œ´M@¨]e‹Êú¿×û_1hÙ¿~‡€££¿ÞÖtD¿áÀmä	)t¿áæ!‡+¿ã˜r‡ÜØ´AGNbll3FGL J0331.3-6155PMN J0331-6155?ïø®&jq?@Œ`Vo'? ~Á¯O"x?bFði?I'¸>žË¸?=A(¸Æ@4?ïàd®¢·?qkßP£Ø?<sNiåì?I‡è)ç?l碙¦?nm!Ñîî?ïÅ-ƒhL<?i£cŸõ?R*›•n›?U9yU!á¤?xޗg÷žO?eSo.²(/?ïÄbgu§n?Uû®l¦zµ?W
Ø}Ï?7Ïy½÷s?x´þ?S^帳ê™?ïñ ntý®?N«^™²Ì?31ÛÿlÂÑ?%y
nè¿ì?Wò¬Epà?KotBe¥B?ïŸQBׄÐ?…õ‹%ñ'á?Qâ)†_Î?_ó]ƒÙá?…ïmæê?ƒßGÚ§Y_?ïŸéKÀ?x§5ðÇ
?Z$9í?` 9n}5‡?"³µhpñt?vRøsºO?ïyÝ!?qå)0Ä!¼?ho§]÷‰é?S?•@=b¯?‹œÞõ"¿8?p*~ÓÍwAGN4FGL J0331.8-7040¿éâí±¯÷ÀD{tÝÛÀ;ç&ďçiÀ=©'^aµ@"ÙJb¤ºà?Î*ÚI7+?ì?»×²?éóœDnÄÚ?ýâ©Ô#Ù@í§d2"¿ï÷[0H¿ïOµIùHV?ïé !óð¨¿èÝV‡Ì¼?Ó¢=ëó¿ÊAÜCbUAGNbcuSUMSS J033202-703952?‹ /?±ä£«ôÔ?_
!C×þ'?|ÖÊU¼Þ?¢Þäþ!!œ?°vBŒ`ƒË?nêÌñ?•
??b³'M	'¸?sAb'È¢L?‰¥ÚqZs/?'ÊJ?ì¶q'4‰[?§«0ý&p?†ŽÉ;Zº…?…Ó+Ò²?·zšÇÌDØ?¦º6â´"ƒ?îJnMâÙ?™noÿB$?	h€'¥Ž·?9ɲ°?«R¼ßpµ?™m"«<Ú?î`ÆÇØ¥?°=Áɼá˜?q%âSÐï=?oZYˆt'«?¬õ7IUK?¯Ðd	~~Â?îÑt£"ø?©Îבgj?w¡Šèõw?—øE»9ì$?ŸéÚ©‹(?¢NÄ£–6?ëOƞ#Zè?¯³k'½`?‡ÌàÇ???ˆ—"#žô*?ÁDz"¹q?®nvûÿr?ì{ŽÄS‡?±0a"­ö>÷†/6'7?¶"Ö¯§'?¼"|>?±œßAGN4FGL J0331.9+6307¿Ã•žð©@Ç€¾À9*æ?d™ÞÀ;ÎÔ°ÆÜÉ@×ÍKͳÒ@4dÁJ¸‹?²vNÜ±œ?¶Mp÷ê@WZYèª@	¸¡"Ä"¿Éëð¾ïi…¿âLð=ë¿Þ[^Ëgqÿ¿â‰Úßµ¿âú1T5â:¿ÔHþ¡†"AGNbll3FGL J0332.0+6308GB6 J0331+6307?ïÈ¡šw˜›?hʕÙÀÖ?@ít÷5?1dú5§µô?y'"2èR??g"ïlO*«?í%ã#Üý?¯yF[Çè?mòß/vÍS?ràlj£@?µáOîÆ?í?®±4·^ÿÔ?ïKòŽl.?'	K&fâ?gÓ}ÜèÐ?fEIlLݾ?"¢1ó¶ÿ-?€¬ªýK?î4îOÈ?€®'ÈĨZ?ƒN)µ,[?_¢Û aœ?§û]";Óï?€ZĚ=?ïsXd£¡?'
‰ÚώÝ?UPu7?IòCu?H4¬lör?i$sâ,?è?¿Ë)!?Ãú§W¬i?O½Å*f?7§–Þ?Íìö^ìu?Ãhà«É>o?î·µ,®E?'¨Q›?p–BIÃç?læëfO?¢|ìb.íU?ì$u?ë2:GNž?Eò¥òÖ?˜ëó>â¥?|¯ZG]…l?À˜{ü¦?œ¹´G•AGN4FGL J0332.1-1123¿îJ¨hЊ-ÀH–s-õÑÀ:Õѧ' ÖÀ<lšu%F@¢Ä—ôþÅ@´L{՝?Õ%
¦w?؆B#æäü?þÚ®½M$@Ž¬7+¿î9_^4i?à°ïÁÄ[¿á¾Jô°¿è¸uAË|¿ïþ0Q×c)?ïÎ0Ö¯ÐAGNfsrq2FGL J0332.5-11181RXS J033223.2-111938?ïρn:×S?rI61lÂø?Lv(?H#HÃ¥?t¾–î4v¸?qNf½"¼½?ï­ÉÛ?'⪕y~8?Z°Í¬2…ß?d,4âI/?aó؄Üã?}º×ãÂ?îäÍqYÖØ?BÅ,Pˆ?†Ì…Ƥv?ƒÿ{
µ?˜ZÁ
°?ˆ–ƉwS?歹ë¹×?g‰E? '?RfÌÎá`>?;n©ªnþ}?ƒ
«fWL?fDú*0Ä?ï«V›ÿ5¼?~l<ƒ±ØW?Yñ<üQÚ?^Áñbgƒ?ì1XÙ?{³¨€­_?ï4zz3f¤?žüÈjæž?k¹Ê¤?€`‹ŒäË?–9€j£¬?š.)€yY€?îk%Xæ1^?—*µUúÂÛ?Žs:¤›_?ŠV£™°gR?¡°ÛÅ,'M?'¨å':?îõC4CdÀ?ˆ¼¤»ªžK?c ìY9)?UìV<'?žó{äÝ!Ê?ˆ"óŸõSTAGN4FGL J0332.8+1557?íËu¥¯¸¦À?È)ˆ;£À;H™Ì¢ÛÀ<ŒÎóº1@ fWÎ.å?úàSý®(?ØÞG ÏÄ?âc¶ˆ½©C@ úÄV܆@ü0à¿íèÐ~]($?ïÙQu=™¿?…Ñe¹¿Ö—¼Ô¬j¿è¦¸f
{¿ïü¬ÄÉ%AGNbcuGB6 J0332+1556?ïÊÑÞON?pk#ö8…Ê?] ².H?V'´Öˆxº?s/E—«¯#?jf"yi6q?ïW™Ï	'?"»¥Ó§$?sò'Ðsº?}52®]?)qR"™?äp¯ùÜ?îð£™L¦?'!e€beü?}¸r\œÃ°?€ú<ì¢?š}pF££??Œ lå?íw^"–G?'ÿ]o|!ª?‰,v^3ň?vl}mpF;?±€ö¸î?''?ÈÐ?ït»| ¦?…©¯Ê0ì?|½!Ÿg-?xñTW¤c?"ÂÂesTê?}zYqƒ}?îMcqOµ?±°8ѝ?Ž6ÀΕ9? ËqØàVl?¨GÜ·_g?©´œvY?î Dàüüã?œú²Ùəî?†Š8lqÝ?…<rÞ*("?¨Y#Ҁ˜?™PŸÙo?ë	î–K0?§æ©Mß?Œ¾oÌG•?…ÞߖJ|?¿ÿ⒠šÙ?¦Žî±(J…AGN4FGL J0333.1+8227¿éðXBƒ«@5IPüqÖÀ:ÀAFmDÀ<¬Š‰[]õ@™Têèí?þC:sÆ?Æï¡
+b?Ëyˆ'!@®ŸÀ@.وœò¿îºadw?ïù·a*½C¿ä<Í`pƒ ¿×H¢L@¿â¦wÎm·¿ïㄟ6'AGNbcu1RXS J033208.6+822654?ï،©F4î?^¹IÈV¦?R»Ÿßth?F!Y+ä"M?n†¦U`?Yp<è"Î?ï³å߇(m?ÊŸ?aµ£pÌ©?khnЁ…ü?}2>‹"êÑ?y'_E?ïtÉV±Î«?z˜'Ê#Ðl?kÙzœ1±?i÷°Î?‹×K¨`a?uǖèqfr?ï
t$a€›?s£ÝNñ?"ì—\âá?cæjç¯C%?";lŠu??pK%^ރ–?﷗Å?K?o=€nóNQ?dGì&$?W`Í|}?z'P¸?j¥‹mn†Þ?ï)ÍD}Á?–)
Ö²r¼?uúKä®Û?€'6
¸©?•GÄ|֜-?®¢jM¦§?îû€Ek<?Š2••§?z@-)ŸYÏ?y^_ªâ ¯?™ÿó²î?"°¬Ÿt"¿?íœom(Õë?)/(€Š|?—Ò1,÷¡?OëÐF¦?ªOð˜®ã?‡q¯+iJAGN4FGL J0333.3+0233?ïóàî²ÀD~~¡ÆÀ;a .QÀ<‰<
ÍH@ GRBBÖ?ú{R¡ƒâ?ÒÁÐÅTÞT?Ôø'Äj'¼@Œðs›O@¨¾vÁ¿ïþÃÎ!a?ïò¦Ey†Õ¿áËZ§ƒ¿¾p¢ÕWŠÖ¿ëÁšÀ«¿ÕÝC<•²"AGNbcu3FGL J0333.6+0233NVSS J033321+023110?ïmyõ(On?¡{"ý¤:?iä­§¸?st|üié?ŽY¿qÁú'? =.™!wë?ïÄ>Pr´(?yªŒ'5?M^ý(êú?W$'¾Ùy?z4ø	Ýh—?uÆPY­?í¸J¿åo?¡b1÷"Ž§?˜y ï"?"2EûÌd~?¨y¡aÒŒ?œ£ð˜U*?ïPH‡'?r#b§µQ3?i®/éRŚ?SyVƒf?'Á6»©?p  þv•Ä?ïg5uˆ÷?Œ¿cű¬?p}qýþ7?oªØ,¥?ô±ü»?‡ÕGúÓ`ß?ïC9%:¢?"§B¯?aïœßiž?oAVa‹‹9?•ZûðH†?'.™³P?í/âˆmCÈ?¢ØCÉ9Œ—?"Y''n?'m%Ñy"?±j¡Ì}xz?¡Þ57ÁÏ?î…äãfc¯?‰sÏ(ÉW4?uç]\}Š"?h"¦{²Ü?¤äÆ/E?ˆc¿i™AGN4FGL J0333.7+7851?Ɲˆ
>â@2vF¿2/À9ƙWTz¬À<f£ÝÀ:@Ôµ'"™€@ÐÞªDã?³PSÕj*@?¯Cûq??øùìU(P@æ ‡4U¿àQž®+w¿Û˜0bôA¿â Ð$p!Ñ¿ÜOþ$ކ´¿á‡_<ü`¿è´À}‰AGNbll3FGL J0333.4+7853WN B0326.7+7840?ïÔÎ÷§õ[?\7˜÷?NkG´~v"?7— æ Eg?qË-Ã0¼?Z•Çø[­?ïÇz;õ€?zÞ튬F½?W	Ìm½ƒë?bP-ß6ó?v€nΊ/?tBCV¡äJ?ï‡-Q®Å?x5rªûÂ]?eZ&ˆq%w?jÀ›y¸:?ˆÞ!ÿqIJ?sHó=Áé?ï\Š€)¹•?i~­Œ˜
?{'©þÝ?Uon®ê¨?‹RL"úH4?eù²ç|?ï§Ú‰›A1?pêŸB"_?`DÞø7¥"?J󵍫'?ø%Úèe?l|¦´7?ï?ÇËÜ?"¥í/F?q,ú*Ê¿?{§UT%];?"»Èƒ@¬?Ž¡túëÓ?ïœ8&ÚW?‡ž§Á½?pÏËÉ­?o+hÅÛ{Å?˜˜†;qYÚ?…Ew~GËÊ?îSVGú?ˆ ]¬N??'Û%m1c?tE '-X?¡Ä-ìÍHH?ƒCW~Ó*ñAGN4FGL J0333.7+2916¿îþü°üHÀ5êÝYÀ9óæí	ƒÀ;­	¾º@U‹DÂ&×?ýV‹@š?­[åÂâØ?¸Ñ|ŸbÜC@‰Oâ–b­@—Ñ)(¿Æ­þÖ_G¹?àµbîᶿޛ¤¡4˜Ž¿Ø?"Š¾µ¿äg8ô=T¿â;ÊYêWAGNbll3FGL J0333.6+2916TXS 0330+291?ïÑÑd>Ìw?pkl¦ÉÁ?Hö1K"¿>?SDÔZºA?sø‡ŸsÞ¬?l \
ilx?ïžýÓø1¢?…jF%n?e·Á‡¨5(?lœH»OµÂ?'Òš"ZÞP?€c #!žZ?ïQYNzâI?Š5ü@vË`?kqr/»?q!	(âf+?'f§ìÓq?‡ÞQP÷â?í'áÍÝ:{?ŒÉ؉kœ?=*¸"?gg"Ó'×?³꺯¥?ŠºˆèÌ{§?ïoÚWn7?‹‹Ë¯?b+ysf?^ކ1i?'3}Y<Ê?ˆ¦Xwmþ>?îôþ1ý0Ë?™ïÒFšY?~¬Ûb3HN?‡ A¡Î?™µë<°}?•3@IFE	?îˍ¤:?–zóÎ¥¶?{¶ù
tKw?€†88·žÁ?Ÿ %XYQ?"½øuQx´?êFW+)h?¡T~¹AË??›ò­%pÊ?'
㋐¤?ÃhN.˜? ì¡¿²üÐAGN4FGL J0333.8+4007¿î"®åÓ{_À)Á%µ¿jÀ:žjÇ7#À<^/",z²@ÅûÍ@@yƒœS?ƃuÀÌcp?ÂK´^kñ?úOfÛl7@…íë*†¿ïôäxºüÁ?ïû+‰>¿â: D®…º¿à¸‰9˜¨¿æX'r0t¿åPJ9ßöAGNbcu3FGL J0333.4+4003B3 0330+399?ïÍ)wÑ%?d†õBXàW?HzÝڝ??
é=§¥[?vkûÇþ.3?bïeí\qÀ?ïÊ}§(?~´}¼œF?F0ÍN0F?RnÐR`n?wû* ñ'[?|\ ®Ë€Ú?ã9B8?r¯IRÝT?]Ó?0<?XÕIÂœg?ˆ¡O¦l?p¾ò™8x?ï
~[z¥
?sN¨¾Rq?vsɱPxË?T<§§•=?™Bê=?r*SM jñ?ï™uáX/?uçh"¶L?`¨âDªÀ8?Uÿü$1Š?…xO¨@?siÚ«±ðæ?ïh8œ¡?'¶êÜY?^¦–~È?e[ gGš›?'"§ô?ê§7ùô?ïŒ%_,ƒ?…»¾Ï·wv?n@Êj-Ü?pؘÿá?™M³3•ûø?ƒ%tTiŸ?í—z,cW¶?Œ;ìm»•#?ˆµF!zä?pph1êv=?°-5jíu?ŠBÿ‰+›AGN4FGL J0333.9+6537?ììåcœ‡‹@^ ƒxÆÀ8üƒýP"WÀ;×ÛIgR@ \@LÌ6z?þ°®‰ç?­9Cm"x?¯j*$@Á@y¸_~@°E
%W}?ìêKBž‹¿Ç
A\Õ¿Ü*¸$õõ¿áÝÖ´¿Úr
žêff¿á!ðÐrAGNbll3FGL J0333.9+6538TXS 0329+654?ïÇ@Å(Nå?']Ëø
…¶?@¨»þë;¿?E0?—ց?zJ…ó¿â?$Ð_ƒè?îßL6'8?¦5sØ©tº?Sç9•Žü>?a~¬â2?¡lŒ5?¥ ð!¦óé?ï=‰í÷aB?"rÒSêL?dØ®d%?fÏÑ(¼a?•³À
+­?ƒ5rqBR­?ïßœ?lU»§@5L?flcÌÊEÎ?F_ö§¶8ì?ŠtFís?kP<`\üÐ?h½H?…ªn½»Ú?Rƒ¹‹æùU?NûG[™Þû?Š‰Å@Zpá?"1‰ñtÓ?ìöqþÂ_®?¹îÜRbÅ?mFˆ©?Zz'ÂèÏ?·c}ØÞõ?¹¥Ìœ•b?î¼ô*geH?§æ¯/u?m@5ä	G±?n¿ùވv?¢\¹øv?8Ì&¦7?î¶\¸40×?ˆÅ£ Ÿ†?|Žin¿_?dL¾à~!?¡gJÅ~­?ˆv'ržAGN4FGL J0334.2-3725?Å©öš6Þ ÀK1–¦ ZÀ8V(LýàÀ;ŠÓ8÷˜R@vz†.?þ§]§{¬?¡$Xyé¥ö?±gýí<j@«BE@i¶ÉŒ&¿Ül—B|Q_¿Ù}Ã@1¿à_ÿ¯x(0¿àªjl…dX¿ãÑ}ÁKå1¿àŸì.'ãÃAGNbll3FGL J0334.3-3726PMN J0334-3725?ïïà)Ã?R?K? V–?%ð™oýá?±éÒ?]™²–G?J
(ö•˜÷?ïÙ%Û(Q¥?ut#è6e?HûúÐ[£x?b0¼'ǵ?pM"!«"|?oàW÷Š×?ï·_,,Ñ?z˜)bÀ
½?YÑÅ]`I?dÈè8þl4?}Ûø©"wh?wð¼+ë?ﱈã‹Lœ?d%Šr;?G[ð'"h?0Yc‰Û°Œ?'%±iÀË#?ceZz…dQ?ïÛo—4?a>ÏöÜ@Œ?/BÖu_V?#eq|È?qNŸÄ=?`¯ý#xËY?ï¨ê³QÃ?†ÃŽ-×^?U¼i§ŠZ?jÓG(Ë2¾?ƒ$Û²
óÏ?ƒ,…ÉõÙ?ï|!äI?'±Ð²Z}?`™ëÿõÖ?p"ù£`ÿ?"z|'‰šG?€y·D+?ïkRîSI?z'_Ã}L?U
¶xðÕ?Cõ樌
?'Dù<?y¿ªÈ¾'ËAGN4FGL J0334.2-4008?îÑÜߝ§ÀK	ˆ MÀ81"+sKQÀ;¶½-˜½@'Y‹b@žý¼XáC?—‡>¸…:?²'T>×½R@œ
²p*5@µ‰ÐMà´¿È÷Œ¾ê¶î¿ÜãÝ Á¿ã"õ¦n"¿âáÑa*<¿æà¹(«¿è à¨-±AGNbll3FGL J0334.3-4008PKS 0332-403?ïò¥³û'ÿ?KôÛ܉8Î?3x¶HÛ.€?&Û\ Ö§?UÖjöÖ+?Hó-ERV?ïÞÇmMG?siÿ(Þ@?@1HsŽìÖ?T¶
j£?m,@Â<Kó?p`aÿd·?ïèý æP?vù `ÏJñ?W4рíz?b.iH¶ö?x^a _¨¨?t/™5q­?ï÷9}$C?5Íkëüáê?!çZ²a€®?Zsõ=ì%?N 4ª++X?3Øàÿæ?ïãڇkl?`ZŽ8^ãˆ?5ôڏËÛ?+'…CÔ`?iqº+"C?_Зpî)?ï³`S–™Ï?ƒÐK$s)Q?PÓê"û?k	Ϗˆ3?
mϯáË?Èÿ^ª?年uµJ
?'½N«àe?]՟VŒr?j'
‹ÑZ?'¸‡Ú£#Ú?kÄzù?ïï¤`ðŽ?M_ßñft?/("•ç<A?!À¢¢Cð?\Òâêá)å?K¹ëAGN4FGL J0334.3+3920¿ï	yHkS¶À*æèÑQ­À:½lŸe‹uÀ<rüp(‡@!"nPj¦'?ý1?Þ<`Ù?¾%vkí¿"7"îfÐ?Ö¨"s¿ë=@3ÈÂüê¿ï¹¾GMò?î÷L!ìŽß¿âZr¦æ‰¿ÑuºÆ"$¿å˜<8d?¥y@ޗz†AGNrdg3FGL J0334.2+39154C +39.12?ïå¬ôÒ®?`D¤m߶Ç?7Ew©'ߎ?12ÍÔ©ûë?gk? ù¶?]3AÌÚ2ï?ïÎíöŠ'È?SC³ƒÜ‹?=Ērð´V?LGÙ»µÄH?v¬»sTÔ¢?€—e-÷u?ï~šªGi?uòöw?Y…ê:í?BL]&žü?(˜7ŠT?u¢
ºµi?ï0´sÀb?uä†û¥Þç?hË^DzIš?Ljµ½ºe?–ÐÐõ1?ucgˏ?ïÒì¦S]Â?kÜBÀØ?FU¸~}Å?:¨ô¢
' ?sÉ3R:$?hِkþÄ×?ïsÆ»¬5?°K•]Rt?R`t]—¯7?bþ%­8o?a6½£f?œ'΁áIº?ïtzÙÄ?ˆ$\:DrÁ?euí­™?bd·ãzD??"¹'ÎÍ?†ÿþ៎?í¼à"'ø?'坙§ˆ$?€ ý
‹(ý?lwÈC:9O?°Û½ØŸ?">¦püôAGN4FGL J0335.1-4459?Èü‹äÀGÀJwŽ}ܤ±À:¹é›9­À<z	d,ÐC@¼ ý¦‰l?ÿ¸ŸõÔ-?±êUéŸì¿R 	äôû"?œ,=mO@û5ëÊ?ïë}[‹¿Ìi"ïî¿âç&J¤‡¿à`ÃY†"¿Õ:5ÛÚð¿Þ`¸vÔsAGNbll3FGL J0335.3-4459SUMSS J033513-445939?ïlÇÛe/É?¼}h9éõk?]EúVæö(?Š«f¥ÅY¸?'¤í;«r?¹qèû¢˜?ïïf5¥9œ?dõ‹Zƒ-˜?'MÅø?8¹¨Tß?^R°žeR·?bÚI" ïÐ?*{\J?'XeA¹6?R&ô‰ð˜?\RåpSÅe?ŠÓÖՄïM?'f/¢@š?ïëèôÿ#•?Bû5«‰ŒU?+ãV"¦({?®ÿ

Že?bXÕ»%2ÿ?B`¹a?þ…èž?´/Š¿Þ"#?[ÓpåLI?ƒòPý¹ø¶?‰2%üoÐé?±Ö˜cÊ»â?ïÌ6ö…?}Ö[Ëfÿ?7Z‰~"Ð?OڻЋ«=?xoLÿŽ[?{ã(¡i@?ï4q‹³}?'U {³?SÄä0Ë?UB§ê2­?˜@Ñ¿@kW?'Jù à?ïÏ=og?]¿®¢."s?@O6Þá9Ó?-tÍÎÔµ·?vWJO;Ÿç?\uçÊ<lGAGN4FGL J0336.4+3224¿ÐÄfñ?Œ¢À2²býüÁÀ9èT菡À;ƒT¦Ë±@ÓÝ@ß'T·?¼éÝú'Ï?ÞV›Ã'@Õ¸ÜU
@¥Í¸Úýg¿¸ó3hãi¿â1®~-,‰¿ë²¶°*Ö¿ïîªm&t?ꋪ=UËä¿ïïë L'(AGNfsrq3FGL J0336.5+3210NRAO 140?í²|þ>›?À"–>è•x?±¡Ùeì¬?À0»Þ+ß?i_¢eØè?yöߥ)‹8?îéþÊ(‹?µ‡¨æ?'%âŠÃ?®¸%…vì?"íš@Á7Ú?¡–_û®°¯?æ;"脰¡?²0`OËð.?Æ
Ä.Àf?­T/À•Ò?Á°1û>"?¨rÙa;Ìb?îãŠl¼'?Zƒª"÷?l–Qÿé½?mNR… HÎ?Ÿûè0dþ†?œ±iÂâ?î;Ê—¦?²Ó~ö2Õ?­†«¿Éc?±·é2UŠ?dYyKûëñ?mèm‡ÚäÄ?ì]øöU!?ÈO Éû?±‹o¨Æ?ÄëåU"Â?§
KC]?­¢<¬2íK?å	Mη?³r½¿l%¾?ÈüZ
èuö?°ŠÏù¾W?ÂßmÐàO-?©ÄPçϹ?êB±ñ²½à?ºIÈ}Âp? ÿ˜ôO•?¨éá(Ñä?µQü!#;?´X}n»€'AGN4FGL J0336.5-0348?ØñÅÌõ´ÀF—ædNÀ;Eag°À<JFu/W@"pø¶4¯à?ùìl5ç?ÉmŒàΌk?ˆÊ‰¦‡hÀ?ÁE‡ô€›?ÿ¥,ŒûÑr?ïþ¹^Zÿ*¿î' ×?ªqDC"l¿¿ÛfwBוÿ¿ÜTÙv({?»±Æ¡‡GAGNbll1RXS J033623.3-034727?ï‡E9x¥6?ŒËþ¼K.Ù?1üAÖ?%Ó·Ç÷ö?¦I¿âd¬?Œ­
h}‡?ÌÚí*?†_ՎôA?\`ª>GXm?f,$ÈåØ?…÷~d$'?'ÏA8ßæt? µT?˜¯htj?W ºN‰¿¡?FñærÇ?¥ü(#ƒÁ?˜´7'ƒôÃ?îZþ~Ô$
?‰®¡òSN?XFçqÉ?A¶Â{L?©àÓ¿Û"?‰§s"$Ï=?îÜ['Òû?Ÿ˜tó _×?=&s§MÌ´?3'#Æ/,?¡ÿùù?l^?ŸwZ<}?ïÇÚZæ?šB!wÏá?cj&U§kÝ?ròŠ‰ÎÐÔ?›™¿ðu'a?—ò¸p~«?í´MŒÐ³a?žðþˆÆ2‹?[óžãzw6?]ø:§,h?±íÅ­Ÿ[?Ÿ
iðÀ*?êáîÅE?¦æG¶»?i ¦…9·?`/Á_@P?ÄÂPXCI?§KKu"AGN4FGL J0336.8-3612?粬ÃrÀJ÷¦a(9À:DՑ—l™À<m?æŸÜª@ȋä¥0§@[Ò#Mââ?½":'x5?—³HG8ñ?Õ螄ºåD@<¶a{p?1‹"G¿æèG]ÿ¿æ¨Š'¾Ú¿ëpê7.j¿ïøp¿…¼m¿ï÷¹_‡¤úAGNfsrq3FGL J0336.9-3622PKS 0335-364?ïãã[ÑÚJ?iyçwñB?OŽúV°w?D$ª¨–.®?d8åq*Üð?hÁ¹9šE?ïšÈA¼|·?‡xÖ@îü…?dX"ç3?qðR"«Ý?"7Î]¦V?€õT4p"&?ï7°A7#?ˆqc¡c]5?q‰°§*y?qôÿÍ©aP?"§‹´N‡À?†Iu]ÝÓF?ïšÅñ'RM?g'àû "^?u€´WJÁ?^~ÌcnX?}ûŠŽ²Š?]׌ò"À?ïÁ)6ô͌?sÁ'þ¥Ð?kxGHGX?gÂÆÛél¸?q¯AeRƒ?kÀ¨ê)?îï–iŸ'?¤Bě†öØ?uÂ˒ó?†Ò5YJ¡?œÅÂC;Pÿ? õ'xD·?îm
¡]w?–bb†ï??'*5â"?~›¢R?¤¤®§qV?"!?Xa?îÞ~€
¬?†ã»²»W?û쥥?€œòIøb?"¡ô=lØ?{5 ÒEûAGN4FGL J0337.8-1157?ߪfï*ù1ÀH
A1"¸À:ž¼Õ,À<_‡ÚTtÌ@,³‹™Q@ž/Egé?ÄaJȦ?§ß"\BÃk?á"Ì`it@Ðú'­Â?î@aNÏpì¿êÈ@Á;I,¿äD³zì¿é¨aé)#æ¿â¨:{üС¿ïø¡œZAGNfsrqPKS 0335-122?ïÔ£>o7¬?sXÝr|–I?@oËÇZÄ?/Ôéa«v–?s gCOè?rþî\emÚ?ï­Gí2'?}H|á÷?W¤¶–ÊR?]°±Øg?¹mÝó¢?x|1À˙g?ï7¿X?†ôgduòâ?iËè×às=?e~˜O'J?•ã_ÝÌ~'?†g~²(*?﭂X¤É?aDQr÷3ø?Zcû¨B'?BÅo
9‡?S	ÑÙS?^ܱý)À%?ï|×(gʌ?‹¾2âÚ?QÈnáp±?E,‰ßŐ?Ž'4†ŸŠØ?‹g'èt•v?ï/NØ]Ø+?—^±Îûœ?cÛÌÆ¡øS?m'šíçW?—š«dÁ‰?–#‹Î¿f?îX¯Xº?–J¾@ø+?x¥4ì¤?nv`žï Œ?§`hºBu_?•F€@LäD?ïcÖދ?ÛÙÉ?r"(Ƒ­?bGÂTUo,?™.{"@U?|¹Pyƒ9\AGN4FGL J0338.1-2443?àñ/OgÀJNœË}AtÀ;r–ÇWBÀ<¼œe%ô†@!óx"9®"?ûp)þ×?ÉÁ`ÝæO«?©Ü½ýôY{?äáý€É¾û@w{	
À£¿ïÜT\È?ïŒD±à¸<¿ÞaÁæê°¿ãáÍzq¶&¿æð莐§?ã笁Ӫ7AGNbll3FGL J0338.1-24432E 0336.0-2453?ï•qÄhz=?·›¡á°—?%³qZœXR?1H™ÕÅÔ?ŠLÁ';Óø?·'LNû?ï¾x• ?{iþζ¼?NÃ
ւ{d?VÎS~?}$b"›?xd#¹À?ïUm¹Û9?"ÏSpo?bÈ:c$?jOLñÁ?"ϼñV}?ƒÃ'9f¡?ï&oœß¸ü?½LÙLäì?aŒOƒÉÂ?M¦Cq†Â?™zÖÔÆ=?®Ã§Ö'?ᅳP4(?uºm©m£z?<Eº¶Î?­?8J"ß@?~n|5‹Í0?uhb¢å?ïCœkŸÐ?š‡œDƒc?`'g1;?n2Ö''?•|%Ÿ´¬>?˜÷^k§5<?ï	8u¨?…ÉÛ\°Ð°?cGŽûT s?c7m'À<µ?šUçNøö?"Øî±2™Y?ít–â•?žE‹‰èI÷?sWo²}?n{^L[2?³%ØrÓ
?žžÚîpAGN4FGL J0338.5+1302¿æZóStFNÀ@w¼Â"çÀ8ÖÛjËÀ;~$–¸=Ê@ K	óô®é?ø"ËßgD?±2jáJ]?Å,Àþ7~@ßZ',•Š@=ZÿU
¿ïÿæj,Ą?ïÿô¬å¦¸¿Ô5Wû"‹h¿ÆÍ7€ÊÀ®¿ßaŽû°åæ¿ÜB"dXðAGNbll3FGL J0338.5+1303RX J0338.4+1302?ï¬ÞùJ.?©ö™1?y<ɘ
  ?¤¬<úÖ?p¶F͸ä?"‰ÆTã‡?ï¡G³rޚ?ˆ‡PIw ?[ÚøÙúî'?b<ÆÓæ%÷?"2´ ¡¶?…µôHZÅp?íM*!?£ReæTV?Ÿ—d&{?˜'°³(Æ?«¦3iœ®?žV'à׌?í:'ƒB¶?•çáÊ6¤À?zÀª.ÜC?b\¢
µõH?´iB"í@?"øUeúf?ïÆõ-E?wà¤'²
?nÆ,½Cs?qÐË$¥'¢?k)Þd"—;?ila-§s?ïç;8f?Ÿ¨³ÐÂô³?r2GøR'?}§U?›#L Ʀ?œQ›`ë"?íÂAcU?¨"S…ñÓ?¢åíÿÿ'‰?ž49½Ü?­
ð©Vî'?¡L^!†?êw·±
ï?¨eçW•?ˆF*1Áè?wfažÙ‡	?Ĝ¾˜'Ĥ?¨aH Pï'AGN4FGL J0338.7-5706?ïÿNéÆOÀGþ+@öjUÀ;ø|·
èÀ=,:ñn@"ANoÑI?úç5ï¦?ËîÂÖSß%?–ï(lZÇ!?Í ÓŠ+<š@.Õ>5p¿ïî4[Q_n¿äùp~î©?ïþ$'ýu¿ÓÄ­ÄsâÑ¿êýOa<é?à@¿ºAGNbcu1RXS J033832.0-570449?îæ¡ç"D?§‡¨à"?^ÎG™s²?g:þJ÷‰µ? ŸoNDñ?¦õ08ïð?ïÃ$)Lvó?x£Í¡Œ?LSõÕ¬?T3=™†Ä?zãl‡Kèÿ?uTy	ÇK?î]íl»¦E?›‡yiJä?…S£[³[Â?ˆÚZ.=¸Å?¤Ì@Y
AÅ?˜"^ùÿm°?ïšÄ$eB®?oFWu`å??Ä'Èny5?5Çéüµm…?ˆP՛؂?n¼FSÉY?îûL9iƒ&?¥¿e‰œã?^æPߝH?hBx#;?ž¨Ä}Ôß?¥075 ?ïjOc·×À?ŽÝ|Œ1jö?UÏBV¿dç?en–…ÅÖ©?'Yhìv¸?Œ?ÏÌýh?íú©}×
,?ž¡É<?8Š?¨©>=­?‡
	'Ûs ?«ëf8?ÍÐ?RšÎð4þ?îßE"
?ª¡à­,Þ?P©Þlþ¢/?R5LEYwª?¡†^ç1¡?[£åƒðAGN4FGL J0338.9-2848?ê#m­Nú†ÀJ"K±¯:À:ŒAœƒÀ<^.bT@&n¿%oP?ÿ…1˜(€R?²#M"M2¿—Ÿ'ya7J?èrŸæ¿@àP64?ÁH½Þó@¿âXœ‰8#¿â@^"àÍ5¿ß	Ñeõ¿Ü&D!íæx¿ÆD
›åNNAGNbcuNVSS J033859-284619?ï÷õߦÕ?Btšñ…VR?" Ðd'
+?!5ÈÏh9?Ooôñ°‡l?@üIíérr?ïíàª,þ?caº–§"_?(¼A¤%'@?:R¡ÝÙ%˜?`"5)I#Ü?aA\#"ï;?ïÅÉn¯œL?gÿé7?¡?K<.l5¾º?3÷¸H€s?y³ÂòNب?g¥ãg?ïåfÌÞ?Eh¾67 '?,%²y‰ãª?A	º4(?hוÜØT?DÚè"icæ?ïîí…BäE?Q´q6™Z?4·ÎE"Œ?&¦MV«?\÷4A2ŸÄ?O£%ñ˜"z?ïȍÔO´/?|ŸS?‰­?7œ7œ'n?Jsr95Õj?z?RpN=n?{)Sc'ä0?	¹^¨?sHçèk•¤?Su®†ÿL?B5œôÆaC?…¯®à¦éü?r©ôv-/˜?ﺆ>?cî÷AZb?AÌG Åp?/=ïeâ?€A®¹wî—?cY9æ)aóAGN4FGL J0339.2-1736?çћ̂W¼ÀIG"#ÐÀ9•²F8ÉuÀ<\ªûÁ­@†rK!œ?þd¨Uôÿ?°ÍÂkØ?¡ØÎbÏ1?ó'
8ͦç@w|üTú®?ëpø@¿Ð‰§»§¶¿áC™b<5:¿Ø´Ó[Ý '¿àÇ7—FC¿Ý6¤!1þÖAGNbll3FGL J0339.2-1738PKS 0336-177?ïë§ýÏ=?T|ƒ"Ý¿Ò?2ý‰BÒ?%"÷†Ë¿é?bI-µä?R¨ñM¤¿?ïà³:×u?o3IJ‡á:?;IZbd‡?FÙ,jÔ:?k㚫Ժñ?k%¼—;kŸ?ï¶[[ÆOZ?gxçµÂØJ?T	7ÌËü=?@ý¾œ¼ M?ÐDrG´?eS±"Åt?ï}ú-qìñ?eÃÀ'®©?_–E·§D%??\]³ÃF%?ŒŽ«Ýq"I?dS"7åÐü?ïÓnÍA÷?jQv¨†‹?IÆÄ%åCÐ?>WcÖ.&?sÁá_ˆ?gÂÑ"6¤?ï£Z›"À?ƒÈþ=¤?IÙvª?TOÊ¢3ôµ?…—»°á-?'Ÿ³pyŸ‡?ïu—Qð}?(8ÞÍ?`	'Ö¼še?YÛIÛtê?Ž—áÉä. ?O€ò\ìÿ?îÑ+ÄÝrÀ?€û¬Bm€?r˜²õ}?Z›ê™sÔm? š-r'Þ]?}¸…߁AGN4FGL J0339.5-0146?ì&ֆ½|€ÀE:h±šA_À7qëýê|
À;gKoj'@
Qg¦­S@ðÜá?'Ö•<VŒC?´Ý)¼<ë@kMHˆ/@EµªœK¿ËûŸú[Ñ¿àÍìlø¿å€…áÖÊ'¿åÒBW"¿èæWbg~>¿ç]™£ª""AGNfsrq3FGL J0339.5-0146PKS 0336-01?ïÆèqÃç¡?à7–Læ–?YFãßxùù?|ɗ†ïpÚ?v:o#?ieMMúœ?ïÅAUŠÌ?€&‰ºPÜ?Pþë]|¢?i†ýFÿy?y6$ë5?z~+õìF¶?ï¹2îÁ?? "!ðøŸ?mÌ÷ýk'Ù?|ZzÑl?t€öú›?t
gÈNC?ïô6›á?@±Äï8Õ?1Ô»ð³w?$G[ó&?Rpcà80;?;é¥R}FZ?ï­µð€?v.7ȱ›¬?S2™e°H´?OZž§rQ?',hT"g?t¡š°¢&?ïPŠ@­'–? ÉŠ!³W?gªuN~›?†¾svLëõ?'ý—"'?Ÿ#ô"?ï£aˆÒ]?†¤êé2,?sÒïûÌÑÂ?€'–~—ð?z|-ì·?}§™0/"?ïæ7ÇÂvÞ?[	D˜Oˆz?CÒФ†ºÝ?;ɼ2ßS?dӄ4J:?W:¸GŽAGN4FGL J0340.4-2422?Æ_ǦGQùÀJ ÝDÀ;ö,A§jÀ<»UãTÏ@ Oa<0?üz0bžZÉ?Ñú¦]Í;?Ù9Ã¬è@$ž¶,?ú©W³è¿ï×+Ë_åC?D8>5?łZ7Ùá¿Ö~œÚñÔ¿é5­@ÀdŠ¿ïúö`™ó²AGNfsrq3FGL J0340.4-2423NVSS J034022-242411?ïš
¢gÀÑ?}´?g›(~#à?`ª ¯çԅ?ƒ–NËRÄ?|	…_YèŽ?îg×Ð6
Ù?¬©ŽíÑ?™ž‹Á ¼?•Õ £&ŸÍ?¡5³·š9?¤Àà…f[Õ?îÏqÃÍÛÒ?'R×ÄÍ?ˆ'×'ÕX'?…¸ÍÖ?™ÈÛ·²o?Š ñlE?ì·ÐEÇé?
Ú|øI? !¢B-Î¥?€90Mn?²0®¬ºÙf?‰°üK?ï©ÙéÑü?Ž¿jx>·?ƒ0(_ÌÅ?|ÓNÖ+¸?"Ä0y£
?‡±æxj£?ì_Ն7o¶?º7"Ÿé¿? ì‹Sç¥ï?ª7Ózí°=?´‹&}R?²ŠtÑåŪ?î+0h[;Ä?™¾g!:'?'á3rYtø?‹³ùŒì?¤\_¾‹ÔP?"o#QÓW7?éø0É?¢¶kÞá§n?¦¸3Ö¤Åz?"½Ÿ¤u–?Âq/ãGˆ? •Ï*9çAGN4FGL J0340.5-2118?ï¢Òj›MÀI–Ñ¿zÔ²À9E?']<À<Ciô`@©÷è‰ø@Á°9ï?ªî^å5?°0Y9(Á@'ÿœ,ñÑ@
Ê*uõO£¿¤øÜc˜¬¿à@úœðž¿äÿT¿:¿åqøÀƄ3¿à]s]Å­õ¿è ;tJT¸AGNbll3FGL J0340.5-2119PKS 0338-214?ïð]·Hà?S¢šQØîL?&.††E?ˆ2›AL?]'Z9'¯?Rr;õ
@é?ïákpD^?n³~UD!ç?;.iY×?Fd›"í¬ÿ?k4IýßÈ2?jÔæ…0Z)?ïºEÔVH?qÏë‡Bj?S՗£T–K?SÈpʪ÷þ?}è
Ã&°?pv[O©¯ë?ïᶍè'Ø?K×»©·0À?Lè!ö/J?3‡kRW]§?glÎ<t?FÊ"¦[?ïÒÌÈý?pÿ/š?<£æÃ@(?2ü¶œ]ϔ?tÏÅÙs8Y?p>Ý°S~?ï°èD™ÚT?† â'™Á?I÷Ôþª£?Y\'ˆ¹?'&q|ñ¢'?"Åsµ«ß?þ쯖?ðýu~?^´V «õ§?Zª=b'r^?‹Ç5fǽÍ?€>ærÍÁV?ﶷŒ¸Ø?h®èÙCì?a׌ãå'z?OdðzL™?{¸µ5ÒÚä?dÉ"×ôÔAGN4FGL J0340.5-0256?áLèvª	ÀEtžý†¨üÀ:ªÏmýÀ<Ybцoñ@'{^p"Ó?ÿøŽ‡à?ˏhc?Ñã<$ôV)?ý
O#SÂ?ÿ‹çýÈ?ïõøÀ·¼¿ãí¥Ùÿ¸…äÛâ>y¿çƒ¿ÝÑ¿å(R. ý¿ïÿA^o! AGNbcuTXS 0338-030?ï
lvd¥
?Z[@BH?n‹
ªZV?fKØÔîˆ?š¯ÒJx?Ÿïôð…?ïê‰mžá?•Q­SÃs?yd_§
À€?yÙXvc´…?–I–ã6¾?âµ¿í¦?î"tUߧè?"Ž<¹Ü¿?"¾ºeë?¦òIhf·?¡™؈?'®Æ	a?셝.ŒÂ?Ž¬?ýº?>½QW?pÿØ<=…3?·ÃEÚk ?‹â•¥­j?î	'§{É>?Ÿzè/©¼?À3BêY?wçØt<g?ªöÈ»ôw?œ8/´]7?ítO)!Ñ%?³j9ÌØÊØ?Žçݵ­jj?•iۙvçœ?°€‹…¤
?°__GI{Û?í>'ÀŸ~? "¾r¡E%?'ͱkuÙq?‰d5¹¿6´?±›êd÷Ì6?›`†j¢<)?è"µ0<̀?£ú°0› ?›–òÒ[Ù?‡ƒŠßM ?ÌLãä?£VO¢‰ëAGN4FGL J0342.2+3858?Ä:™)ÃYÀ)˜øçÝÊKÀ:QÝIÒÄÀ<9à+Nbd@9ºZ.t³@üº€™îS?¾–y(µÖ¼?–Úâ}ýˌ?Õý†þâHµ@NžT¿J?íó
¾¯}²¿æ4M¯¶;'¿å¼ùðòF¿âˆ^Þ²¨¿âÞsV–¿ëšŽ ¿"(AGNfsrq3FGL J0342.2+3857GB6 J0342+3858?ïúÍgɵ?1€9šÒ^?îf'`Ùm?`J;&Yw?D
ý"™,¸?/Uô¸Ar{?ïÞ*Ä5	Þ?‰TJkDX?)?†¦£º?D'þPòC¦?p ¡•!só?‰7Xa	?ï¼SîÈ'Õ?k䜶}T½?Tiݒ5'ß?[¡wB±rU?|»';~<»?h̍`?ïëÐÆàf?CÂþ"&ª'?"pYÉ]?Ï÷DqÒ?c/à& ›?C"	!ü`"?ïö§:°ÄÈ?@éKq76¸?)e˜ždŠ? ΠWa¾?O	®bPÓ?>3|~ð?ï¡F|Ī?ž:ԇï2?7N¥Ùð:»?Ol\i7?‡y=2ÚV?Ùúbì)?ïˆr†@‡–?z¨ñ.¯…?a–z(ÏZ?fõ`@ú ?‰}¿ã6¼?wf£$–8?ïÃ	])"f?e£$÷u?:ât¬ôR§?%1D''@?|Í*'c[?dÒ#Â]£@AGN4FGL J0342.8-3007¿ÄõÑË0·ÐÀJ>U⊤3À;\ù1¯¥uÀ<è~ ïÏ0@|ØãÀ¯?øï»åüj?Ý儠¹?ãJB¾ìdm@ l‡י@Úën"d¿á²ý¸ýâï?ïÜ¢ÍõÁ¹¿Ô—€DY¿×Aß3ÞL¿ìŸ_¬8¿ïòÛßå-lAGNbcu3FGL J0342.6-3006PKS 0340-302?ìñíP®vÔ?̎o˜æÁ? ×Ä0™ñ?µjН*·?°³v˜i?Ã~iêvÎ5?ïGÆB"?ŸŽ…Hq?tÜvÀÖ_?ƒð¦úâÖ?'Ðסp?˜óm0Á$3?î4¶‡Õg?™ù
&ìï?'}É>f²?‹QÇM%™?£v ÏÁ9?"iʛ…‡2?î"SR|Ð?€ÿǓ*~T?†ƒñ;Áø?oÎHì»"?¡)ÒN{j?|Ûf‰@?î/¨¸¢h?²Mž+j5?›	á°R¦?¢È	3ç
?ž‹ß<(]?¤ƒ;à²$?î}O`‡ÌŠ?¤ 
ÕF<?¤w¹`?ŠÍKo6'?£ã Õ¡Rc?¡ s?¢3D?íH(£À†?¡7ÈOÕ,?›k'â8ä?'·C±W<?­Ç¬µ&Ô/?šØˆuc?í–0
cë¸?".Ø'e?…ã1]Þ?Œ±®Ø'ñ?°'gm ?'š*š$²QAGN4FGL J0343.2-2529?ên*æ±OÀIÓ|ÌyÀ9ÊdpÂà»À<d‰éù-~@Pm"½¿i@±oɼw?·*Aë1è?Âo'Ÿaµ@¡âއ	t@ҏe?Ô‰[l¿ä\¦(ô¿æ߆ôÛ	¿èq¼Û¾¿í2ê£whí¿ïüwIãxáAGNfsrq3FGL J0343.2-2534PKS 0341-256?ïóåÊ'_?K@ÖRÓ5?@úKÄÒ=?8s®Kw=?Qi6\ò?CŽJ(ÿJ"?ïéjöª'?iþCôíÄf?1• ·î¥E?A èšG?dbe-‰Ù'?fíížF" ?ïÂr -ò×?r"~|þp?Wÿ#À_½?MbM±t*?xÇ,|CH-?qºš ÏAÀ?ïöqÇ)[?5èb¨¨?3~g­½!?C•œg‹?L|'q£¶,?3;V¥K§?ï楻æË|?VˆÉŽé
E?U8JÆ	%¤?IfÁh©ÿ?]|=	k#¾?O¡å§8?ïÁgãWíl?€"¹XÅI¼?CÓ$ñ0ÕØ?S®éä=o?|Ñ©À­(?~¯<°jÚ?(4?|"à}¢Mã?d½Œ"߀Š?gfüàÒƒ?"-Ô¤ÒÉ?xR=vmn'?ïå`˜Ø:?XbegCIA?LuLx˜×?=p;9äE?cßLŒæ¤Û?T…Ôýà €AGN4FGL J0343.2-6444¿íÈBYÊTUÀEÔa¿7¸ÔÀ9y'S+ ?À<Sá,Ö"@ýt»¾³@	…º¿"?¬IƝˆ¼}?§áUšç!?û'YY7©º@Çl½Ãp?ï ±ád"¿È™òD€"¿äCN¾ÿږ¿à`)k3TÁ¿çí¸4Sſײßð–AGNbll3FGL J0343.3-6443PMN J0343-6442?ïñÀ"°%Í?p#ë€åÃ<?'Þ@s¼b?Aªá h?Yƒ¾
ôo?kñr‡}«†?ïå~Ö0	?oN¿
™&?5òFۄ?FQui<ÈF?hB <ߥ?kàó•LyŸ?嵐Í7­?€†r¹p¥‹?Vß80/_?aÇÐsÖR'?ƒû¥ºÓ'Ç?€;Ê`?ïç÷ulL?G•WXÂ
?CØÿ°+ÛÁ?)°°i?cKD é?EV@i%i?ïéGJí9?et':,΢?0Lî#"»ì?!ÎX}\÷ì?dæ*è[Ö?e
©‹b?ï²Ï @
?ƒ'ÊlN<?G1ìη?ZÍÄ)Qm?Ú$ÐÏ"Ù?p€—$T_?ïO–¢ˆƒ?Ö%z³±e?]ØUÚ«ƒ?S9k'?"/¦SâÜ?tè+ÅM?ïÁÍg§Y ?fˆÏ]ÿò5?Yó‡ý?HÁAô¶ç`?xœj+gW?cKmBùÑÊAGN4FGL J0343.4+3621?ì§þ4+‰NÀ-fãOÆñÀ9ð¿§J\EÀ<jÃQ#@®Uÿfþ@€W$'°?ĘvßE?ÃÕYä!þ?ý&¾æZ<Œ?ÿe*ß|¨¿Ð"á+~‰¿é¹vCS;ç¿ÖÄO»)6Z¿çqÿ Üï¿ç
J5®7¶¿ïëa½µ,ÈAGNfsrq3FGL J0343.3+3622OE 367?îU_Äqð™?žg‰ˆÆD?si 8…[¸?kÈ11¦@F?¨<ß­šÅx?œƒø‹È?ïvŒýæ"?Œö1>E?pFïærßG?pÂífO‰?Š9H–´ÇN?‡øë؎sŒ?íÀíYùàE?œ;o›ë?'"ð$z9«?ƒPÊ _?ª§2P¸"Ö?"­01ú¾?í
6
—Í?DzáÑt?'ö¥F°??pžíA'–£?³lþÿü"?‰±nÐÀ›?ì åRՐ?®÷ÜÅé-Ö?‰2Æ,È֋?¼7+˜?·ð Ð8¯?¬ðgÊ~8Ì?î)ºr›í¡?¦S^áA?Œ#¢ßwü?'`Njkæ?¦[p?
ò?£r¾™@I?ê·'3 –c?¬x¶w?¦-þrºœC?:ߌÞnb?¿/Ç)0G?¤ÓyŽ\/É?éŒÒ—À#?¡™pBÏD? ÃAÂó?ˆ4¨Ð¯Š'?śå[0t´? &á)î}AGN4FGL J0344.2+3203c¿î¢­ËšÀ1ìP½‡µlÀ9q±6nQÀ;5º‹¨â@ÿúPh£-@qÅìÞ»?בÁŠúD?Ý×°UÁG@"˜Ã°ÄY?þÎõü›ò?陊€!"¿¿T³.@/¿è«ÆÑá	¿ë!jÃQ#¿á0–5a
Ý¿ïí%g˜•ŽAGNbcu1RXS J034418.2+3209030?êEièÀ¸?»ÀINܽ?±æʦú!¼?¬]/¸­Å›?»íæ%ߖ?´}¦±]š5?åäyùì?ÐKN
G?ΐO'~6+?ÍÍõ)?òè?³¾å3Ä?´ë+Næ­?àáeͱ›?²=úS†?¿›ñÖ¥a?¥&Gêß¹7?ÖV7îó'?°"†¡´	 ?Ånrø"Ą?¡å]‹x#?Ò·A 3g?±´ºc<,?ᙇ¡'5,?°2,0d‹?å1_jëÿ?њyù?¾cãv©Ìå?¶½ºqf±?Ì}HÆÿi"?Á`Ç
Ú¾?Ù7mc&Ÿ?Ӏ,óJ‡Z?ß&茛Ú<?Ô®—`7?¾†©k¸y?¼‰^§ÄïM?Ú
z–7ÿ?´•íÊز²?ÁÞl5ÍF?©,¶™?ÝONá~N?³ÜÚüòK»?¥KûªPŽ?Œú='?"¼?ӛ8 Z}û?¿Å,Žqr?äÝ£õ;A?¿(Ï[a>xMIXED4FGL J0344.4+3432¿Î&Vš°4À/ô‡B_À:ÿ@ÿ¤À<ï< @!v_[…6á?üÊÙþ
·y?ƎDÑÁ(T?ª‡1j…@?å‡q^-O@WDŽ¥J¿ïö«!ÃI?ì{Ϲçû?È6â?OÌ¿ÐÑLŽNý¿æ¼Áò~7>¿²PÂæ$AGNbcu1RXS J034424.5+343016?ïè)¾Ñs?_'†CÀ8?'žêȱÅ?Èt?
?fqõË$ªO?_$ÍðÞVç?ïئŸ¼sc?ukcWë‡Ï?@­ä—Îo[?S;ç ®¡?q–óDªé?s·$šv‰?ï†Ö'ûiæ?tÙp¨kdï?YWZ"úR?UÁ²lO?‹sÿ$d™?tB^ô}þ?ï…+£qà?t"¿ˆA³¤?fkWaoÂj?J´—ê¶:?™a路0¹?sB·Õ*Ԕ?ïØNð ]û?cعëú´™?9€ÄúÌwö?-à†
d`â?r@{Dí¹b?cáÅD?ïŠ>ŸU¤?%Tï0Æ?Vt3`,?p³"mîž?Š­)ÜVß^?-'Éì~¶?ï:ñÃ.ò?€HÐɜ™¼?a )¿?`ç|†zaR?–€|A;?~oe1íÁÅ?íè#Æ6cG?wÚkÁ¦?u<šÖQ¦?eÅpÆf?®Ö@*FãZ?Œö¶àdIÐAGN4FGL J0345.2-2353¿ÅÑc=ÄÀIj³=¯øÀ9@ßìdAÉÀ<Dªùš‹@ƒ°f·š@G÷`MÉ?ªÐÌ`Á5ë?²¿ïn¸D€@P<Íæ¨@	n£Rÿ•¿×˜ÑÞ«Ü¿â™ð‡Ôö¿ç¦]¨R¿åˆGä¿äÑTá®±.¿ïÿù_|è3AGNbll3FGL J0345.1-2353NVSS J034518-235218?ïàŠl*¹?ƒ|üŠ"•ç?@2Ä™''?^ÔY$–t?khâ¯ô#?ïMg'<?ﱃ)Y"o?ƒØé&{ë
?Wâ-}ÚÕÞ?f'†Ê9•'?€¢ðâIU?€'ݶ÷Dè?ï¦+W³+?}gÄ݄ç?\Œ¦¼Ù$?h,Ja|4˜?'ã¨Bi0?y¦òøl?ï³`"yÖ?ay:8?kÄ®¥lþ?P¬ÊèâÓ-?xm¨þP"c?ZU®xoó™?ïµD™HL0?'Vø'?OT°—ia8?I'Ÿ‡?€¹Ž™òÃ?kÇ÷'?îûâ9'ë?¤7mN?p»[V¯?‡$'•Õ{?œ{ߐ<Ü? ®NÈä½?ïDW͓¾†?Œ/Y¾Ii?c¼x±?g'˜‹(?"ýwCì.‹?‰ðqi:0q?ï0·'㟢?ƒãŽä©?"DG"ktI?rrÓ'ø÷?Ø2k?{4*îWïPAGN4FGL J0345.5-3301?ïD­. ûÀJeè'%À;(*FûgÀ<ÇMé—Þ®@åכ‡Û@lCõù?ÆÐ=…³:¿'ÈZ]É?Êá|œ³ªg?þ|jvìEŽ?ïÇ@f!¿è¢®Á¿ãq•+uпæ£Þ+™á¾¿ÙòÑäcÂG¿ïó²I"ÇÉAGNbcuPKS 0343-330?ïÇÄëT?mƯýt??=öþ¦¬•Ç?*È`…Æ?z>'~Z?m$xÀ¾(?ﺉþ	õf?zM¹ó1Š™?ReX[ûB?XÑ<œ<?~!ªþÓ{"?v%ψs?ïQk]×Õ?€²´2x(€?jmD"»-È?g¹lXOð¬?'"ô'!œ?~½S¹÷?ﲃô‰?`_{"þ/?Rˆ"¼œaÎ?9wìpå?,£÷3…?_èõ|5\??9?~îC醐V?Qç¹3|'?CÖ+/g3?‰Ø£"b;?~…šohª?ïQ•ü×­?–Þd6Ò?Z0'lUë¦?cgÚ®Y"ž?"*=ñF6˜?•\/H4Û?îàòEžÆ?Š=¸S`R»?rð*°äž?kÏ:³­³?Ÿ%´Tï?‡´†L8Q{?ïåئ8¨?& v¨3?ggÙ~œD?XîgÔ1{?™vIµ
 [?+{bÝ©ïAGN4FGL J0347.0+4844?똅â'Àg|¯Ý©À:tü+_)À;¥ðFN™@²Æo­G@©âå=?É?:èß'?Åu°†E)?ù´…xze!@Í~¦#?Ë?æm®YD>ô¿çnµŠè¿åK—"pî*¿ç—IBi1¿éöÒÅ4R¿ïþ YQUAGNfsrqIVS B0343+485?ìÆ0ls5?¿Å$aÖ¬?yl
æ\_?€˜˜
úå!?¸8uÜ áT?¾HcJkø»?ê­«×?·ÑeN«!?h]ËG¤¬?lÎÝâã~Y?Äêj#±¾?·"ç80?íPèÝ? •·‹ف?'1Nœe9â?vý^0&)[?µNëlía?Ÿîâ«ý?îT{q)R?'uuœ Ç?x´\…qz?TID6¤£?¬$,·Çkµ?-"·9?éx¤#Ú?À:Ç­²M?†<øÌ"š?{)Ĭ>î?Ê6Mâêy?¿¸÷Ø¿c?㒩ïìÑ>?Çz›SÐY?{žÐñbÄ?‰:NÛZY=?Ølu¥"ň?Ç?DIÂ'?éSqA5Õ?±æ"à£9?•m~–Z‹A?Šðbò÷+?ÈýgÁãÃ?°o;ÃË?êÞEvX³?š~n×	wß?ç ¼ÿ?q@*±¿3<?¨{|֝å?™:õõ:)GAGN4FGL J0347.7-3616?窅ZzþWÀIÞÿ´€¦À:Жï›-îÀ<¶¤À>I@ý"õ•Ä@"÷H¡Y?ÇàV
??¯¬3á?0Ô?á|tŤº@¼dkd}¿åÎÃ|Áò~¿áŽ®žä\6¿â÷®aÐ*¿å°B½ê±º¿ä•^Pp¿ïÿð ¼x—AGNbcuPKS 0346-364?ï÷Có—3Z?Tºqü×·?ߧ^Ž+ü?doÚð?OÔ<Ôªk?Rǖ»n"±?ïîÛEiZ?d¬Ï)g
F?&à–‡åõ—?:œÖÏ×܇?_mb䐵³?bx%ðCcF?ï©Í_U[?v["ã÷5?Rü©¾:Ç×?GÈùät¬?ƒ-ï.>1?udäGFe?ïû[ŸO?$¥èoij[?*,¿«û>ë6ƒ`gÐ3?ANà'9s ?$@žç*
…?ïîk|OÝ?l]þ0o¦?&ËAÆ5?5€;{†?`|இŽ"?iÃ(¬šð?ïǀ}§S?€"‹øö'6?7Ü)…Âüa?Kã6&–®?zÂ-·Ë?M?~ξ`˜²?ïe›ÉÈ?'«+üHu?aPáçðK?eáµ±
 +?'"œÇ}Uâ?Qšú¯o?ïóž,ü7t?EFêuÙ8Ô?ëG"Ó×?À¢éq'?Wdñ	?DñÚ]7cAGN4FGL J0348.2+6035?´³ Ž£@?Fí$[)À:""W:yÀ<H§+R""@!ú»+Ìw?øê`üšò?Ë!¼•?ÈIÕ·3‡?ö
ˆºNE?ü%1uBø"¿Õq7eGœ¿çåaHÌ"¿ë¡h?¯mk¿±"ùF¨Zý¿¾‹$ƒB¿ãēBgƒAGNbcu3FGL J0348.4+6039NVSS J034819+603509?è0[ßÇ?À%Dgãéõ?r˵[#4¶?fÁ
ÈX?ÎìàåÚ(?À!Nsl?嬞UYèn?Ær‹@n×?‰°.ïGD9?JX}joþ?ÓÙAÞ$k£?Åò±½¹j?ëá öÒ|1?¥ —8Ì?}i)Å_ƒ?v¿J"
W?¿e·ûë…?¤‹¾• 'g?ì±æ,c~?•yÔ,g'?vvÑ=€Ü7?g²–†çÕ°?¹	a‹ÊÉÉ?"ýÎ#Ccó?Þ7sL†t?Å`Kç{b?…mÁÅè?84Q¦ÈÐ?à<¢Œv4?Åx]cf	?Ú؋6ÕT0?Ç!IYmã?'×ë[O©?›¶Ô¦¦?â#¥:{k?Æé¶ý؈m?捞ÇÎ-?²iS¨4Q?Œ×Ì0úܛ?…ÿÖd{)Â?Ñÿ6a;a?²»æÚ?æÉþír?°'ß+Äàâ?Œ¿ÄÛ.?"Īaæ?ы$*Ÿ'?°Œ	QýMIXED4FGL J0348.5-2749¿µóª|jߝÀIv†œfÓtÀ8!ײÙÜÀ;¤ÖO,þ@ž4ge¿Í@³¯Yõ>Ü?™9Æö*?°(U3¹
@ÂܱF^‰@ qÛ	¦qï?ۜÞ]	¿Ý s]Dԛ¿ãÏwÁ¶™¿âOðِ¿çs4_Ù'¿ãUOwÅAGNfsrq3FGL J0348.6-2748PKS 0346-27?ïïÖ¶âQ?OYˆ¸f'»?6½sæ ú?)B}£â^õ?ZÑ$A1î?LɋœÀ?ïé]Eo9¸?kïóŸGÏ?4§CÂx§?Y4Æë­ª?d
Òq@œ?d•·ÀSË7?ï¼oYÕ†?z]Fö•8X?WÄ*¸}?`,…žÒ\?{×M¦»?xýK~®ß?ïþÛ{KÀ?»#D²h">Ú¾¾W!—ˆ>Ð_wŽ*¤e?!xϘjg]?
ÃóÕÁ…?ïÝ%"#±?hód»f?6:ãá
ù?.ÓeO]ˆä?p	ˆOÔXy?g
ÊeÙF?ïËj:lž ?~çyP'1?Ac	€<!?T'°Í'Ÿ@?x¢»W?}c{-Õq¨?ïŠñ–ìÒ7?ˆöÈk5¥v?bh8?ç»?q¾EU3µý?ˆ©Œ=ÖôE?‡šç!ŒÂœ?ïýŸÆŒõO?) |‡ŠpÉ>è>\q>áRmšå?2=bœIQ?)³¨¬Í1AGN4FGL J0348.6-1609?ïÿÌeÁbÀGÐqÞi­CÀ9˜®Eù•À<Lso"
@V0S.ü@¥M–Ãü?² Êzâõ-?¯²1k

?úÆ`¼Ù9Ã@…‹TÝR?ïÿµ¿â'ºí§7è¿æ¬êÿ½ºá¿åО~蝿Þ5xó0䤿ïÿãåîAGNbll3FGL J0348.7-1606PKS 0346-163?ﴀ»&\5?ŽÞÆýÞpA?7œQ[V"?CÅP«Y!â?'"îÿG?Ž5èŒtVº?ïãM Osä?mѱX.?7eÇ;‡¥Y?Bûc 7öÖ?iŧ"'Ó?i鏧ݒ?ïIaÄ|W{?H£úôçï?ua¤ˆÊó?'ÒFŽ Àó?'{^Q6Vé?ˆªò¥c{?ïÜŽ'J7?N?î{Ýc?Q$û@;ª?5p¯X÷?kdó'8ó+?IÀ£xk?ï y·üÜ	?Š|"@¸X¬?AÏDŸ«?B…¹¬'¸Ò?†Ä·)?‰Ú-+³í@?ï¤éÌë^;?Š',ûH?GÐڞ/~ó?V/MʵÁ?…HV'?‰{]×<5'?îöÐ& û?'%Œ¿\	?wœ©Öìøõ?€_í%/Øì?›>ÐÇÄj?·å™9‡?ï¢wàÐÿ{?lMuñ?fõ™¬²M·?SP½"!w?¤¡hҝ¸?h
ÅIÙdvAGN4FGL J0348.8-0828¿ìŸ5Õ¿ÀFU•:À;ážëèòÀ<Œb¥Æ!@·ÉI	´4@Í6´ÇóI?̲fnžï¿qÁŒ/U‰?©}GÔUd@Ã3ºÂ‰'¿Ê¤©;¿ê'Âó/7%¿ÁüA""´…¿â=OG"=¿ë&Ü"U?x¿ïý—"ãwAGNbcuAT20G J034845-082422?ïWÆ2~ØM?TPpM?ZTò0˜¨ö?P¤ÃzZèn?"aê3Æ?r•›9*?ï«åyÊyê?ƒ'í÷–,X?Sïô€®-Ö?ZÎ\q«v?'ˆ¢üCÝÐ?líÚߘ*?î÷D™"?'€ÍO;˜?€€Òxc\?'ǵAè?˜ÍîfζÊ?‹&×·	âš?ï`
½¯_?o+Ԕù>?Y"GË¿]?Bˆ®f$x?'Vª40.'?m¸g2'¿/?î¡<°à]"?ŸÅ㰆I?mC4ä2vú?dºÆ3"S?¤¦Âæ?žJ*fHù?ï3Ašmîµ?—¾dR…¡?^0¹-b?h¢ýèmþ
?—´Êå{vA?–QÂðsÿ?îjqs=?•'Y"j"ó?'MZÞR—?ƒ4˜­EPø?¤Åp걌?'L`1Â:?îanÞû?ŠÙŸ––?j¿
ÖÀ?_/>†y'?¨=!MÌt_?‰ð¾.ÿeßAGN4FGL J0348.8+4610?Ñxjfóv|À¨¬\ý
À:Œ|¦CÌÀ;ã¦êºô]@7Â4moð@SÍÝnÀ?Ü»"¿e=?çcÖ>»@
"x'@	õ¢š¿ß!Ã~ðK¿Üò{}Nà8¿é‹?äœw¿îÂˌZ춿ïΌŠ½]Ä¿ïÿþˆ0»ŠAGNbcuB3 0345+460?í¬êð,?²3s&S«î? KÓُ?¢ßJðí}?¥+M?©õ"t|²6?á¡l$¸¾?È¥=ð..?­Ôꉓj•?¨¢—Ú|¸¸?Ù3Õß3ñ?ÅЕ™¯¾õ?éšØ]ú‡?¯^
Â
Ǎ?²ÌOú>J?¢Ì·;0¦¾?Â#l¡hðÚ?¨Aàˆáþr?çi;άe?ªÅ𺒸?¹_Ì™PÆ?œRËcrŽ?Å«-'f™‰?¦år•[·Û?íK!k¿?´º{ÆÔ?£]>¿ ?¡ÃD'Cü?§ð°ÍVl?°&þÇÎà?ÑXX
Tžµ?Æa͉z'?¿'_íK?¾''£½8?ãnè	XB?É|øAMZÚ?å¹>¸¸K?³«ÂJ™ª?»Ì"r>?§CZÔªP?Ë4½ˆÏ?±wŸaVG?Ø¥"Î?´Æ&H‰É§?Ê~#˜ÑS?¹L¸žª?Ú¸Þ+L'ˆ?¾JpÞܼ&MIXED4FGL J0348.9-4859?îïڈC¨CÀHÌM©>êÀ;i%ö3ÎdÀ<Ù=x0"F@£Zì4Ç@«ôz¿Ö?ÁýHëC¿µ¡ÙÀ6wœ?óÙ¤ì³òá@6ìÕ*ê9?ïF®€žÐ¿âH†`Կꟴeͺ3¿ØÜ̉°îJ¿ï÷b|×Â?ïÖäH•AGNbcuPKS 0347-491?ïˆ/}µÒ?­Å<#‹?eÏèwÛ~J?x+ñkÙÀ?›Tüûvú?¬h"Î?ï®TíuÂX?qGÌ5×?ZÃj=­ë?bÐ?¤ÙßG?WK†7?yLÎ<@?î'.'–À?—w
.ŸS,?oÃN¹–x?pG«ÃÆF~?¤âˆ+û3ý?—FO?ïÂhsž?axÃKöÎÖ?XGq&àsÜ?EŽ¨›cÅ?x¹êM5oÓ?^b)3‹¸Ò?îÀ]A"b?«Ç5ÑK¡9?|á5pä§?"@|_ºV? ^CÅ.?ªÊnëÉ{Ú?ï7àâ¶÷?™qϳÙw/?dÀJzýî?r÷_äˆX?–'žÉÎ#?—%ßþüÌy?í­ÏXd½f?¡¸2úàÞ?t?Ý©«˜?sœ'ëUF)?±MÞ}Ô?¡[¡Û?Rè?ïRÈÃ?…vx¢ì
6?wìÿ]EèÜ?lŒ#ñ>³?—'Õ̔‡{?'ø¼RuՅAGN4FGL J0349.4-1159?äŒhv¿'•ÀFÚ$5inYÀ:E†ö(æ©À<R°«#@ öODú?úUPÊï$?Ãþ>ß¹¹u?°'_~ØÕ?ìRjÑ/2@8®©K=k?Ÿd³dÆÔ¿ç\ðû¿åü½€S¢?ÈS™Z.Ÿ¦¿àuïÛŎ¿ÜìCŠ™AGNbll3FGL J0349.2-11581ES 0347-121?ïÙz¶±z?\®–"ÿí*?5íh!…Õ?#'r[òÒ6?qãλã?[V˜òŽ€?ïمDÔ?q²¿W³¹??¦^͍‹r?IlpPAþ?qBøkŸX?oJ£FQ'.?ï`D-†?€GAW˜(:?\éìÜü^¥?DNMؖs?'(ÝUn?€…w
O?ïvgmw|¹?n}!ëlˆ?P,wuõ?94ÌÑi 0?0Jàîp?nÁ?ïªÒ1n?¬?uï/¿]'ö?IëuCR´»??ºJ¥¨ä?ƒ¬¼X'Åd?táùX ¡?ïŽÇìÖ?‰«»×Ðð?H%˜åKù?TÉ]ŽFñS?ŠËä÷9RŸ?ˆ¢Aƒ¹û'?î¸Ú¦L?4ø²¹
?hÞÕl:\9?aHɌI?¢ñ!×ö^‡?"P¡~?îªßû"½?‡õI©Ó^È?cEûÐ,?VÖ¨ûWÀÙ?¤§Dwà)?‡¯ùh^†AGN4FGL J0349.6+2410¿ëÜbTf'9À7°³''dÀ:·ÔÌuŽøÀ<8.Ýc@°ŸÑ—ö@Þê· ?ÒBh$¬‡³?ÜV܅§tN@KŒ@Ã@	ޖMß²¿äïÍug‹¿ÞÓ0~¢ó5¿ëÙúnƇ¿æ‰Éb4'¥¿ð?ïÿæj,ĄAGNbcuTXS 0346+241?ïÐß8ÄÃ?‹=¨Í¬*G?h'lѝ•Ÿ?xï××Øož?fù[B;Nä?ôW^˜] ?ï*¡æ^6?˜_jŽã?•´ÒAH?‡ùƒnqé ?'àèėL¢?$"d"?í#MY? ´ðz5'? ÉÂ-?™ŒéÇ<? ˆÕ*³@?"pœôbªÿ?î÷šÀ­|?'^Ñ°Úþg?}c°´W[?b²Ú…ä…L?™³»·YP²?±%0vúb?ï¼ëIJÝÛ?
Ö\4Š©?tËn×çƘ?{HÂ4Å
ú?i}ØÙW˜?oÈ4"М1?í÷~ãF?»4©wT—©?¡ØÚ5æÍÇ?±WB"'¼#?­·­ÛäÐv?¯irÝo?í¼Õ¤?m‡? óÒQõTÑ?Ÿ.ï;=—?–2MRb0?¤›.j\?–Zk•×œ?ëd	N)Ñ?¦à'Îê¡? ÄM"m?ŒêXªº?¼Ó펟{Â?¤y;¼Të¦AGN4FGL J0349.8-2103?æØ£÷…KôÀH"tûTŸ•À9€'،À<·ÀÌ
Š@ÐÃAØ@¶øº'`æ?«Û®¢Ñ?ƪ[É)*@Aél?Ä;@w¢jxš?ºËŐÃ\6¿âûMÿm'¿æÊé½ôAÜ¿èÂ:ØC""¿ìd3áƒé¿ïü³µ¥iAGNfsrq3FGL J0349.9-2102PKS 0347-211?ïx¸ù[K?
ì×Ît?~Äç§ÎÎu?tÙ¶àkv?xþ»÷kÏ?uÝÅb17Ú?ïÌ<V¿Í?zCþZ'
Q?L2üÖ?[ŒÁŸM?vv0ÿ¢?váo«?î°E=Ýí?Ÿ¼€¬ì:Y?–m7!:žs?"³,è–Vï?™œÀ8Áqã?–l\Íõç"?ïìÎ÷§õ?G|õ+‹(#?Iy×ÀÇ_?5ˆ²¸
?[v¸\í?@,²ùEü?îðˆõ÷,a?–_ý>û*"?" eCYN®?ŽýÒ¿…/?Šœø	@ºh?†u}!í$V?ïuù¨'ÈÚ?"ïë¿?c'ÝÚê†l?}JHnÞ?œÞk²_÷?''ƒ®=?î6ìpÅÕ?¡Ût•b¯?•cGB̾?•‹Þ±£?¢_•R<W?›@¤©ÐÅì?ïʈåÊÓ+?e…u†#?`èېø÷?Rsw<¹?rG†Å‹Ù?_¤áËà\WAGN4FGL J0350.0+0640?éIèº0ÀA"ãÞaIÇÀ;…BêÊÀ<–'nQí3@#Ç£Œa¢²?ùN"wÉe9?ΝñµaÌ?aoyyWsž?ž]÷íÛÕ?ý—ÁREG¿îb,°b2û¿*Ù>ís¿éTr]•‡f¿Ð$÷0M¦¿ÕÝìd—¯4?Á].Cà)¡AGNbcuNVSS J034957+064126?ïŸÊQ-«E?…ˆ3‡Ø?1­Mâùb?(_±r˜1?‡€@g'C?…açO³É?ï†Y/?'&ö¹Û.?aßóD¡m?s­š¢lÒ?ŠØÜ?Œ½@<Ûþn?î&JRÅ°à?£õÎs¢t?X$bÉm"?EòY=õï?¬ÚÁ¬-&?£ô֚Ѵ?íà‡Ÿqü?›hüçÉ\¾?]{á0\Ã=?Pš;éÜÆI?°…Ó€½w?›h)9|?ï5x÷Á?"Ñj‹ý[?8é?RdÔX?0²‹¯«f¼?‹ëXitŠ?""ÚÛåÚ?î™6xÉ%µ?²«
Ì
¸?o¯/S7ß?ƒgÚY{:?¤q¥|ÚNÉ?±òlÄç_§?îA™éSHÛ?ëÍH;¼?[êU"Mû^?Vx'v~Ö?«½ã÷?œÞ(@›8œ?èȍ—¥#?·®^¢ò?ur:5U)W?vb /òV?Ì27Ïhø+?·NNìSAGN4FGL J0350.4-5144¿á=B‹j׺ÀHDââ¸Ç\À;ªœ÷,À<Ç÷øʂ@ Éh»€I<?üªzýÍÙ?Ã:h[´×?ªà#Á¦(?èÛB±Ux@žÞýÑÒp¿îÔ;kç?àÖD°39¿ã&…¥ÆΆ¿Ð¦c"¥¿Ü¤ßÈÒí¿Ú'Z›WûAGNbcu1RXS J035037.0-514457?ï𚡱?IfN¡2?(c91?»T®äð‹?[Ɂ蜼Ý?HXxâ—?ïÙÖv]™?pä_¶˜B?< xTÿ@?Cž¬9ì?q¶0WÉ.?n°LÎñÅ?ï"æé}~?k.9ûْž?WŸªÃڛ?;,qc*Ø?‡ÒP~Ïg'?j
nóÖÖ?ï°/žºQ?_Äõòë?Lç¦õiž?27Ö×à"?'%Ý™ÎF?^ög݀?~?ïåÜqõ)§?V;Ø÷''?90Lé}ØÏ?)kŽ¬vÜ?fý"|[X1?T¨·Ô#!?ï•ÛŒ¶ºÅ?†Ç>'§)?J½EqÏ ?Uª#V¬?ˆèÀíGK?…­+ Fü?ïMãLëì?zñ7(X?aŒø`vP?XMš*ζ¸?"=ñî"rÃ?x3íÖ"Z?ï%€Ïb;?{€©k?a·Öye?R•â³Ê?™ö4éÛj?zbW""­AGN4FGL J0350.6-3226?êìî‡K}ÀI"ìé¢ÆiÀ;ØÚø»À<ÆEéïƒ@½Õ
8!Ú@ÀRP.ì}?ÑHµüPÈð?Ï¢$Ø|ƒ?ö!‹»Š…*@3I!ßÏ?ï­¾Ña‡¿Ø؄{zIÈ¿ã<6¢(‰a¿å
pᔅ¿çב#'¿ðAGNbcuPKS 0348-326?îô">»Ò?ÀdòÇÞ7?wÜtž,7V?šJ.–N2(?›vZ÷³°e?º"ž¤Š'P?ïêÒ«ÖT'?içBÃӁ?0F¾G"ö?E-¬à¡ßL?c$|G€D?f#ÛjŠ
'?ïo'º˜?"ÂWëÞ¼¸?kR3ÕÁð?r'\㬟r?a"ŽÌ__?ø¢è?ïôøÊyì?6-·Ä`a?àTŸF®?%Öû\'Œ?Tf/ôG?5rz@³FÖ?îϖj)r?º'Eø‡»¡?h{Žž˜L?™ÿ±âGš?ž3×¼?´p"c±¾?ïÂoè›4?äъ#•h?9צZŠU?KA"›5~?}U͉¯šy?
±=àðJ?îÿoÚ¶øÙ?ø9z'Â?tämƒã8B?yÃOº™>¹?šØéA Ôä?ŒthK‡¬¡?ïâôӕ؉?VMPó'ø[?-ã^‹œ?'^Ó¹ˆ?k;)©"­?UßQµ‰²AGN4FGL J0350.8-2814?äŽYW'Á—ÀI@Ü­¡À;;y‹YÀ<¤v¾£>^@"ÒB?úkKøüր?Ëv5{âÏn?¨g=beø?ßUŽ7ï@;­$æ¿<¿ïÿm¾Ÿb†?î½µ7"Ñ‹?É®«d_1¿èÀO`c?Ñt¬¥:¿¿ãÎ#¯1±SAGNbll3FGL J0351.0-2816GALEXASC J035051.31-281633.0?ïÔMPŒ?€dXNàŠ²?.r]ºÆ]?&ôÈ~¡Æ}?u¦X3)?€Kº¯¼
P?ïÒâ±Ì§t?yd5‹´rô?C!é'Â}?PÄÐa$ZÅ?t*"!³)?vJî^ïƒï?ï÷@=ݱ?:—KMÀ¯?`µ¥´)`?`ä^Áé?*cU庯?ŒØó?ï{=¥ŸXÃ?sQ¦[4T?69o‹5:?-*L©*??îaÚÖõ?sJP.4Q†?ï´Äw‹N?x'€¾uð??0¿wu¦?6Ư‡ÓÓ?ÖŽV€¦?wýcâ¸Or?ï‰í3l
?ŒÐ	d¥–?Q¾þ¬µ?f©B7!E?‹LÓJóÌÉ?ŠmÖáèV°?îj‹ðÊ¿?–#RYWùÖ?g
¾Âïc†?hm®f?§æ•6®?•µ 	•?î Yªså?'•|Ã8é?C]=®x4?D/ãÍÈ?¥¬ð_4T,?'ñžK+¹AGN4FGL J0352.0-2516?âõ·^wÀHÕ³co;!À;R>{fÀ<Å憲6I@}pŠìÙ@"Pi¤ßH?Ó°°!á?·óÔMŸ›?䦸ÁRT@fA'šÇ—?âd"¿éöñL¿çÛBEÈa¿Ïˆâ|·`ª¿èàYTÔ¿ïúÅÞÆõGAGNbcuTXS 0350-253?ïÕam¥—K?dž¬-èìù?FX«•9³?7øf@N?rŒ=û¸?co½{kÉ6?ï· "¦îõ?z"ùWân?Q›Ål&	?VyØØχŽ?€buvÛ?w<ïõpÚß?ïoæc2®?wŸÉ*ës?eœUñW%k?f7³È\a=?ŽŸQªÇ³@?tmO2õû	?ï—+÷eãÆ?e´©±'øX?[´'Õ
2K?@{jTÒ7Õ?†¾qÈÍÂI?dù÷X‹º7?ïžüèH~I?z ¶"Ï(k?T¬Ç5î€O?HšYä†?…«-)?¤?yqU$ñ?ïHkܜùu?•u%N¡¬?\B‡,cD?cÒޖ=è?•0>òœ$?#$>ÆÖ?îü	¢z?"ä	üÄfk?n7ã5·Ïg?j8¹Nž?œ¥bpO­Ä?ƒwõNP?îÞ&Žµ?ƒ.Pº‰?m¤A£nq?]óo¹m‹? KìÑDù?'üç:ÐÄAGN4FGL J0352.9-3623?ê¼3Ô\§åÀIYJôðØEÀ:øº˜â›À<uä;~[P@!@iGA]?ôÜZ>9÷s?Ê^Í?äF'?Ó7þ(Š@	™N?Fg@µt«ùm•¿í·4µs¿ë¼=¾&–Ã?æC¼ª R¿Õ‰Ïa§Ñ¿³`#%¿âh'Ü\AGNbll3FGL J0353.0-3622XRS J0353-3623?ï^ÀTÄR?€ bˆLËy?\š"›]?S'Ø&Á6¡?…'ü²éWå?}fzÎl?ﺜç†?|¥8Ó^?PÍìÂîu?[ÙmŠî?~~>EÿÌ?wäÓ,L	$?îšB%êJa?"g†nf'?{áÕãð×x?}ÜÇ6wð®?¢ß¢çpóû?'l¦ÐN?Oq#Ñ?‰s¥`™•4?A':"³{?3ÉW¹ÂA?§3P½ÇF1?‰T°U2½?ï!¦œ¦-?•n öÄ?m˪
Dšk?eiðôÉ9ö?˜%õðÎ?"¥ø#rö?ï4rElƨ?¡B'U:k¢?_5î}`z?g)ì•‹ˆ?—~Xb§? ãM"HÑõ?íc쐮ÛÃ? ãnÓ1Î?"{˕y«;?…C "Õ?²Q"kù?žèVAà]?ì×E÷†	?¤ìn«v"?L
ýôš8?J?ÒwO?»É/Ö©¼Ê?¤ß+ÂFaAGN4FGL J0353.0+5654?Ï0竗ÀH@¸ÌŸóPÀ:ÚH¶RÀ<VÅßrÂ@ jÞ~¥øM@CÂb¿'?ÀŸR–$ïù?µ´"K æ?ó5'éSì@ŒS'Þí¿ëo>&VV?ïå…?ðZñ¿Ø½ây1o¿ß,'Ûç¿ä'è̱¿ä61_žv"AGNbll3FGL J0352.9+5655GB6 J0353+5654?ïØ4Gbóž?`Ù6­³!k?<Q£)?½?)+Ûű‰¼?r ËoßÙ?`²ªJ"?Gëjá?ªE^
d?SÕ;;Vv'?cø˜¿¹È?¦X¦|¹·?©\¿Øné?ï4…hèªW?'›~™ã"X?fÞßPŠj?Xð5B9-ò?–®w""á?XGÌhÀ?ïk'èô˜?h^"£eá?dè¥QzõS?Dz3€W?ûÜk¢Ý?gF=b]?ï´ÃÀxol?rwñÇa·®?MTµ&®@~??Kێµ—?€ùČp¼?q…^2j'h?ëÜV ªÎ?¾ZÅ»Ýw?ll
/š?–-•Ѧ?À÷V'á?½µÜI±=¿?îM'™ísÙ?"Y+<Z)?uéɛ¶•?pÆ*DïŸ?¨i0/¦>?'ÆŽ€r|?î–uBªÓ?" eÈ~*ö?x5ië
?a‰OÒöó?£'	r
œG?ƒRҤ°AGN4FGL J0353.0-6831?ïôáªÅÀDbŒL˜_À:r)ñkÀ<qä"rÁ@!ñnmpñ°?ú.kßL+?¾n­¡},•?›¹·Ç,#õ?àáP¢"ϳ@ó͞Xñ?ïT{昿Ú{´Á¾%ë¿â'OÐø«x¿ÑĪ¿[Ë¿Øše¼Tº?•©˜5ÁXAGNbll3FGL J0353.0-6831PKS 0352-686?ï†>n¶Ó"?½EÎÉÚ³?I%ø c»?J{&JÅ0®?ŒÞ
mßZ?A0—®?ï®ô™¼Ìq?Ñ-ÊÒ?RÑ'k³?\½…%ÖÆ?è¹}gÇS?}Iv""‹—?ïªnþæO?"Í(tC?i¹çҕ™D?tcɗÒÞÎ?œSu'\Uå?'xd­¹.?îÓÈOî?'K1†A?iÖë¨:âK?Q(ÙbéL?¡0"À"nâ?'=ƒç?ïFóQpàé?"À©]Cîe?Zˆæ˜û¹õ?^¢žÅ_+?•yi0H?'øü¤­~?ï4î5l\?"¹WÂ71??_Ø:è«ôê?iÂ<G{a?—dµ§»G?'o½Öyn¸?î("-U	?š_¼s²?q¢aÂã?xpCö)0‰?«ú¢…ìâ™?š4ô"
?f?ì£Ì­'&?›˜}îJÿ`?€–° 3¼?q'Šëy]Ö?¸ÎāZ?›Ù±•AxÏAGN4FGL J0353.7+8257¿ìÈ@">Á@6Q?´‰À;X®í¾µÀ<¿í
´ôi@!Ӑ¸ŸnE?ú"âÀ*'?Á§¦b)ë·?¨¦ÜOKÃ?éÐ_Sw¡@à[\È
¿ë"m‹?ïýä1m`V?චpMoõ?£S=ÏÕ|¿èšˆҜ?·ÊùŸ$QAGNbllWN B0343.1+8247?ïåèˆ{J_?dW`'uµ?LÅj
±?SѸNM†j?bæ1Éåào?`"ï&é?ïÐA¤*J?}ßJñ'j?P·¿º4­¨?b-cß"8?s±†DÝŸ?wX¬šJj?ïPFð»z¦?†"¥ùU??këN3fú?rímñ;\?'"$ƒ™²V?ƒÏzÛJ4s?ïS_#.¶Õ?t™p*?oKJÓ¤1—?[]\&üJ?'ª²Go¾?rPþ¿iø?ïÔñökÆf?i#&¥Ð€?`KHçD.C?]ݕ^®Ý?jÂÀŠ™S}?a¬Æñé¬?ïzÀªYÁ?+aîâ•D?^·å˨‹?i3áIםŠ?ŒÆÈ1ú§?Œ+¡>µ?îâÖâ­è9?Ž»w%U˜ñ?rž'¨lò?ul³Xƹ?Ÿ"ü
¿÷ ?Œ!ƒ¿Yõÿ?îr*+‹? ݸZäx?W­å é?x´äçT?¤‡tâýa?ŒîWà1p AGN4FGL J0354.4+4643¿½ÄM¯úôÀ"¬ó±³À9,ó*.§³À;˜ìÿr;‡@@õÜ»'M@*º:#?¶` ¦Õ?¼ÃÎ!`£@§Å¬G@(BÒ¸t%?íQ5aáœh¿âY>?€Éi¿èw
bZé¿äœ¼cÈý4¿ê§l ½$c¿ðAGNbcu3FGL J0354.1+4643B3 0350+465?嘆ŒÒ>"?v"Öêi.?PTNíÒ©1?E˜Srœs&?ƒÇ'ëõoû?t€&*?î<†-0ª?­³•5Š:&?QáÆÈhœ?^ÛV+ör÷?«®ÿ'…!?­\où`È?ï'áEæÐ?Œx»½*ÏT?scQ	((?x:	*û?–E¯Œ ú?‰Ñ®°mv?ïM*S¡ÎØ?kÓöÊ:¸ñ?q /+¯åÅ?P¨¼œ²ä}?'ò©ÈiOu?hi`
;¡!?ïsµÚB?›QHÕ®^'?aÉ7&ìØ£?at¡Xÿ?¸ba½íÞ?™ÀJpè¢?ëošäa,Ú?¿‰ýp¿[?c ý‰Û[?uOï"Ut
?Áóxž!i?¿S›f+
Î?îÅIÞùӟ?–˜‹lå?¡˜ \¿?'¨µ_­˜Š?žÒsTáXË?"3¿'ÞØm?íþÿ­}YÑ?‹NfØ`°˜?t¸Œï9?r&ž!t²?¨²×^$?‡éãPJYæAGN4FGL J0354.7-1617?áÅFsàUÀG)l?Ä;.À:û|üªàêÀ<€ž @I¥Î0O(@×N›n…ð?͆-—¡?³ÓÄ[d*?áº}ibD@"hMò&N?â"õbîâ¿áuҟʋ)¿åw©Ÿ¡—¿ç‡¶"v¿ïÿ•Âû?è½hvAGNfsrqPKS 0352-164?ï÷ù
?A	"´ç
? #P ':?
,Á*a?L÷czw-??Gª¯ï>?ïÎom\`?vºS(i&?F÷qÉÃnY?U]?jˆèÒ?uéZûºÓ&?r9ÿĈ"?ï»qæLOº?i/ó‹ÿ?T:hïC
?BLQ¡º"Ç?}8r¤@žL?h¡˜Ont?ïèîí˜t?FI?(÷?/×#ód8&?d½PHÓÄ?e{:ËÙ?E6ðÁ?ïî»ÐâAd?UÀ•è"Sh?+¼7bö>?!÷½ÒÂçš?_כ4\Õ?T¨ˆ³¹ô?ï…b@£†?á =;Ú?R–?Yø'û?f5½ÌˆÀ?ŒT§òÙÄ?‹CÈe?ï‹göšŒÅ?v¼ÆàÂæ?[Ï9<x]Š?U[¯Ö®`?‰¬Aóí?tÜæ͸ZÔ?ï¶zzfðÇ?h&SLhn?D§Ù—n¯?5˜Tf'(;?ãß÷k™?gžOÂ#;DAGN4FGL J0354.7+8009?ª'Öä3@4á?J˜«À:[í£)æÀ<–!à$˜f@vlÉ×Ïà@SR"Ã?ÀL"½ê[Ô?À¦ÿVýé?ûpû€>~Á@tP¬ñT?â­ž´5§?Öë©|Åñ¿ã"_½Õ¹¿åv·'"…¿ä»¢£-—¿ëKf/ßÁœAGNbll3FGL J0354.6+8011S5 0346+80?ꇳí
Ž?ÖY™m"›?Nof²¸?§Á"Íôæ?ÄÏ:Ö?½?ÕÇãñxö?ïéhušq?h\3ëëz%?8þQq½'­?GTyY~:´?cwÀìÇÑ?d`šÎè¥Ú?勵ÛUYV?m—öâ?Wcjš'ˆ?[œ>0Zš?ƒ£¦OïÞH?~·'à0!?ïúÂML[?+¤+Ó¾Æ?>ãô¬·2?Ûxõ¸?Aî4wDÿ?*iþüŒ¯?îÀðßaá?ÅÄ­"6*?OCÛ³q*?|!Oø
1à?£tÄûœ÷?űdjÒu?ï½ý"ÉXØ?Ú!?Mõî,Ž–k?`ÅRHŽò?}BwÅó?P¼ú}zK?ïiG¬¼áó?‡Ñ»Îùç?aસ£®?]'Áκ?šõ(${#?‡lÚ9kj?ïñѹ_v?LhܼT?4ª¢-¶
?%Ò¼vâà?X»´6T,?JXXqJ§QAGN4FGL J0355.1-1841¿Ùß*¿¾"ÀGËs2'À;?¦½oÀ<ÇQâJãS@ Êæm²¶?ý6Ó¼)ç?Ñkúú݁P?À!hE
Ñ$?짧¯i?ü¨ÚiÃh¿í(¾ÐŠÇo¿ì	| ºu1¿ÃP"'5ú¹¿ÕEM\T>Ç¿ïхc¯˜?îÉ,«AGNbcuNVSS J035513-184309?ïÕ'jþ?jĆyû[?<Êifp¸?3ù"ÕzØÁ?sŸÊωM?ipÄæ‡ßŒ?TÔ÷?±¤nßÀ?_¾eß`€Ò?cx¹ž=4?…$ÜÊþ?|ð
²À?ï1!ô¦?‹"4ðç?vÞö¿Uö?zZª3°\°?"$	ì¾?†¼?[Á?ï*¢8ù?y½Ñ—lÚ¨?_ÄÏ&Ày?N¹£ÓÁ?˜¯p*s
?x\¦û~$?ï«vÑÌ¥?€@%©™¬8?O¬d¼¬25?H¹Ú^µ1ð?ƒ'…N4Ë¢?œìPõã?ï2°xЙ?—+6¿£§6?h		ùûÚ?pú"SÚ?›˜ˆ±ñ¨o?•—·ßXTP?îÎPAOÅT?'g!À…?u"׍˜?zØffñæŠ? zëNZ:?=hdo°?íŽQGMúè?—­Ÿ²è©?o—Í&ÿ?gª' )?²"'Y,Ø?–è3¿üØúAGN4FGL J0355.3+3909?좠-SíŠÀ&uš¶ÐÀ;gÐâÜÀ<w´ÃÁ‹P@"­e«£?ü¤
5ãè?ÐáÛý—E?¤l…~	?ÙuJÅK#??áÀÛ'£H¿ïêu¿Ÿ½ ?ïþÒn¥Ð¿ÐœEÛ×V¾¿çšãEµ¿½TfÈ{"¿àÑ(l0AGNbcuCRATES J035515+390907?í²¹Çr¬?ÀQáQǦ{?˜TJÔmH?¾õYÄþˆm?¨ª>"<¥T?«xæ_‰Â%?ênp÷l'+?ƶºö¥R#?‡PÜ10Þ÷? 0¼áGX?ÄÑ._¨ â?ÅÓÇ!š?퓫#bcU?ŸH¹q.$?"ñXYô˜?‰W–|Ê$(?°Ä…—ÌF?-	™?çªè_`žâ?¯×_uL‹?•D;œ<Y?ˆ•$]æÎ?Ϋ×|ݪ?°b¸³,– ?ìZtE!GM?¸É³4?$$k<`?­TÁ¹£n?»ÛÒµUH?µ&ŸáÑ#›?åc8KhÅ?Ò1½gT"?—
ҝÅ?¦ýËÍK?ÓÈ-E³hx?ÑÝ1×Çi?ëÇ#'ÄQî?¥?û.O?†ÆW;Ý?†é/6¬íè?¾îÅ>&ñ?¤|½?Zù?ݽ‹Z€mè?ºŸîîñËñ?ŸæÊc‹Ìš?š'o©† Á?à"ÿz/W?¼­€E#kMIXED4FGL J0356.1-1329¿é`\'{hÀFq[ÕìÀ;,ÓD¶vÀ<µ}¼Ä@´HÔÛ.?ÿ<r\=îx?Ñi·¿Ža?¼nvÖ 2¥?ëw "~–@a[0RX=¿í€
Fªß<¿¶Ê=ü9÷È¿äüYòŠÌ¿×xXKo¿àKs2&Ä¿ïöÐâC6AGNbcuNVSS J035611-132908?ﶺªòm¬?²} ¯V}?G}x»(ß?wлlÇ?€Ù…+ö@u?±ñC%xó?ïÉê~Ûʎ?t–˜…äÛ2?Dn&G4c¬?M§Á¶»ô`?x|ûŲøø?rEsif›t?ï‰[T¤%?ucïè‹ž?Zâµ!†?T©¬}Ì/€?ŠW~ô³?ts_Åب?ï›â•û™-?d¨aû¡
L?H|•g®?-<ÒD=øã?‡…µ_á?d-ÁÁ¤|?ïÏÈ[è£?…^"Ü4/?;™­*ÖhÖ?AjÌÌ^ ?v·ÂH?"ó†Ï¯W?ï_	ò–?òñۗCh?Sí€Ä?^$::B*?'ìÝoyõ?ÚᒠŽÓ?ï;4©ªÞ»?LüöH?ba­Ý±ì?RÃOõ?–M5,û?}_–ñM$–?îî:Á5Ú?'.—ô1L?Xß2‰£Ú÷?J!Éøv? X²½¿'?'zÃNΌAGN4FGL J0357.0-4955?Þ¢O‹ÑÀH	‹`ñ²_À:˜WšÀ<žßVø4@]ÁÒî@¯!Áçã?¶Ùã`·û¯?·!ÕgÐô¥?ÿ3;C£@^ÎTsö¿é‹fe¦Ò¿Ñy‰¤*¿âÄãß»¿ã™ã€îR¿âĀÍð¹¿êv›r·®AGNbll3FGL J0357.1-4957PKS 0355-500?ïÛ³£
¿9?b÷§€‡ÛÉ?F¡¯0SÑ?<*K]Q?n£ñ8…?`ÈfC%x›?ïµ	)Izr?€Yâ;?S€½ÛÀ"?WNÓû´?€Mž–Ÿ`?|¨íç¨?ïkë1րš?~ŽÊ|F<Ç?iæšb5=?lXè߇üm?Ž‹Œëª@W?yŽúÒï$?ï›Å7?b"ëØSZD?lX™ÿ	ë?NHÍøf›¥?ø‹°ås?`
Zé1=?ï¬p¦'¾Ø?t:‰%q–S?[¥` ¢ôù?NË©œ…áÐ?o*aÕÁi?rIÏ2&ö"?ïN{'?¡f&†­?m°Y'zJ?½Ÿ`í$?œ2º•Ò4¢?ž××Õ¯îq?îÊ۟½8õ?¨äÊ¡L·?}¨^K>?zÂ
çt·?Ÿa¡ð%"—?‹ÆŸ~cqå?ïûí»?€êo7ÙÕ±?'‹'áÿ?kOˆ#[—?–j@x†•?}3GæؖvAGN4FGL J0357.2+2320?é`ûC
tVÀ6zÞÑ·À:ŒÄ¤	_$À<Legbå¨@ùþ«@ÿÉ^ƒC?Â8‰‰V*"?¨<S~"j?çسiy@ž'¯jfP?î0A`ó_ß¿ßztÛt/}¿éƒ1èEÏ¿ØӦύ¿ä¸é@ ¦¿ëL°/bAGNbcu3FGL J0357.1+2325MG3 J035721+2319?<ï±?~uë	½ßÅ?TÑÙ´	Z
?EŒ¨òٛD?ˆÂ5ŒWPo?}‰º¸m-?ï®õ–%¾?vÌ9øt?V)9'õ'›?UuR¦¹½N?}'>¾Ò?tI>ð¦%?ï_°«oÊ?|˜õfãý?iV~6ȱ8?cb÷¶xT'?ß/ÜÙ¸­?xÇ&Î( ?îëøF]™?r§ŠU&u§?zg|mé,t?Véoʅ C?›ç
<iíÎ?qrñÉû}?ï3y­Òý?ŒÚñ‰·Ò©?k†DµD<?_œ©±!E)?– ÅUsË?ŠÖcãs?ï‰ë?˜`?•v)Cv?l\êx?v(ûÜá>?™-W
¯¯¦?"³Òsãy"?îˇ(‹8?Žª#+]ŽÂ?u,1´µ?k›U›²? ¢^:•J?‹Œ‡ÕzZ	?ìý·Ù¡ê?Võ¬«I?'¨y¹ÝåW?v­Üó9¶Ä?³h(«)jÜ?´SòˆƒAGN4FGL J0357.2-0319¿Æ^iž:y_ÀCÖb^™éKÀ:È5A*l»À<]IfË@!›ÖY¾bQ?ú³Qf$!G?Ç×&—ïJ{?Ã
pÖ×½—?ýÅÆHNMk@†¼
Ý©"¿ïÿ^Ê¾¿ïƒƒwï$æ?ïÿ‹Á>Ï¿á§Áåèý…¿Ó¦¶ão+¿Õ,0àr›ÿAGNbcu2MASS J03572609-0317596?ïpêqV/?ŸV¾¸Õ"?Hñ.͉ð?XOáŝ€?'(eÔå?ä÷>¹K?ïœër¡ª'?…U±'}©K?Xaè"·I?`kŒó;?…¸æJ~&Â?'ž	CU!?îûíƹڤ?Ž¼C4) ?X0^ÐËÞ?UàÑUau*?žÿAC`4Æ?Õúta´?íù™Gup¬?Œ×½w·u?R5¬zhò?Et0©æC?¯Ô¾!¨
:?Œ´TY>LÑ?îÍCÌwV=?š3ž'°O?[¡Þo¶?Uâ
¥©Î?¢N´C%!?™" §
¢4?îø‹ÖÒ#?¡û™‡Æ·?kÙ†6i4?‰¦äRÒ?sdîńª?›K :¾/
?íÆ4™ÝÇ?ygè"U?ba@èu›H?_ÏrhX&-?±;Q)‡E¬?m×;>.?êÖ×[WOÙ?¦hî¦ÈH‡?a¶µ½hä?`ÁKIâ?Ä]ǹñš?¦TjòAGN4FGL J0357.6-4625¿âT¯¸GÀHd\6fÀ:äÜüŸÜÀ<Ò´%t@ô¦›µ¨™@³'[·¶»?"xŠ«?3?®ªc°y?ëGæ^d%@#®ýY¬?ïíZPü¿ÙúsCn"³¿ä³R"ÿÝ~¼¨š¿é"a å¿ïÝDuAGNbcuPKS 0355-465?ïÅ­ø c?gҕ.Î?Qëɵ벵?Aɕèiç?xü¶–tâ?e…Ñ-¿·?ï»RÉGÿj?xÁ¼†Ñ?PˆŒÕ࢐?XlÈáí~?~4x>•eý?uIö+àj?ïsJŠ	P-?y¬«f@ê?gs礰¡8?h¥+!± Š?Pc"Y¢{?tÿ±z…³?ï§x"_æ?aaQEñ:?f¢rsùk£?Eêû
¹Œ?€yC§‡?^"¨'u³?ïzá4ã·u?~A/?ȕ?f¼ÜâhY?XÅ?‹˜{Š°Š±?{yáz|E'?ïM¥¥Òž?€N‡þ?]PPˆ'<Õ?e$>¶7¡º?"ˆæF…h?ŽÖ˜m'S?ï
"?EC?"ù—Ž°/?r×½"i?oúPšu'?š~,3mH?'=óéL,?ïf2õ1?}Ð6
)˜?~&r'â?dâñdü?ì?–ñµ¼ƒ%?y¡qOµ·AGN4FGL J0358.0-6946?ÜÈêŒr·ÀCÛá2µ^òÀ<'³1fªÀ=Šlê&3@˜<%u/'@|x £?Ý}Œó˜ép?ï>ž¦Ÿ@ÍýAÞÌ@…*ÁõƒO¿êÝSb}£š¿Ûí¼[t'?–"MWÕ1©¿ã³_¿-R¿ïüz¿ï—7z>ŠAGNbcu3FGL J0356.3-6948PMN J0357-6948?î+®y?¡Fˌ?)˜Ô_¯?Š«Ï)²ü£? ÃɜU[ˆ?š/a+°ý?꫉B/®?ÀŒ•«‰—T?¶4×`5ï?¶Ìå¬ò±?´nà´‹%?°2ó%ßµ?êø-w¡;?«ò™²eÉ?²Åf¥,s?¢y&ô•Ñ?µy‡Ú+9}?¡0¡ýN?ë<‰y£C?¦åGß;%?»èºÄ"Ö?¡z¼?¤eóOȉ)?–Ó²ñ¹©?í1Ÿà—?´‰-¿£? Ä†brJ|?¢gÍBP@?¬X@û÷?©²—§q·?ãÒèûV¢ú?̒¸‹Ä'6?ÊpÕI·É?Ȳ"ó^ÔC?ÆDM=[¼P?¼JwaO??èïB…-g?±A'°á?·s;ËðõD?¥ÊM%[Å?À‰X?§–‡xQAÞ?äAkù´rŸ?ºP<ÿöÖó?Ï% +6Ã?¸aK¤ a?¿ÖTòý?±aº	o£#AGN4FGL J0358.1-5954¿Û	U`§ÀF=žbV6mÀ:ëIBi1À<Ïs]Å­õ@oéò¢t@¿Š:›?Éç<t$•?ÁŒwG4G?ñíÏ`ûÃZ@oûe'?ïýfȋõl¿åÍEbàŸè¿â˓¿å­÷¯î¿ëÒEb	àT¿ïÿôw5ÁƒAGNbllAT20G J035814-595233?ïq]í¾V_?€pU1óˆœ?fd¶Eþ?_†HªÐåì?Ža.ߊ–?}=LI>´?ï"U¤™ŸE?"KM'œ_É?c'ÿ°Q§u?búâ<ÏU?ŠÖçTxØ?¾®jÐÈ?ïPµúù0?‹ù(ê<ÆÆ?zò •e?}+Trk'ü?•Ôì' 9Â?†'>"¾¨?ï]ߍÞiF?m=²€Ù?w)î
¯8?T«HPxSÔ?Œó•/ÊÑ?i'L/Š[?î½ÈRi¯F?˜‡~Xr?®Ì²þËõ?v-ä«Ä÷? -¡@/"£?•@±®µËÙ?îÆÿ[x³?™íãÚ?r+2:¿?zg$©»ü?¡MI«añv?•ïAåÕ;Ä?Ã3Æ×?"‰*g…ëÕ?€&ç"?î³ÛóÞð?¢Ì]Ru֌?î¥Ðä¨n?îJÎzlU?ˆ—]erè?Š¯7,ê:?rÖY·Ûá?¤§J•Ò%?†¯ï)?ªÀAGN4FGL J0358.6+0634?ÝÆ]'+À@Èك"t—À:6
fðÏáÀ<
$ÜX[@ê+‹p@¨÷ÛnP?Ç.ìË?É1‹þ¦c¬@¯/:€.@‰!.-?åkì O+¿Ó9€TN6¿é°"òsP¿âü^pпïÿþˆ0»Š?ïòF~"…‰AGNbcu3FGL J0358.7+0633PMN J0358+0629?ïâ"/»ë?bÝn]¾:¥?XU³5V	?SpÎZ$¾m?a²öÝ£{ô?ZòùÓ/X?ïÀÙzéü?|òuU¨
C?Qñ`D@à?^>ż™?{ê֌¹î?x‰À3½kä?ïG±tטX?‰Ùrì0M?y{F^"?}̬kƒ[À?ªÿÞÍd?ƒâr¥<›?ïÅM
0Ù?^æÞíõà?N'ü'¬?4F¿Gmeù?y‰\#Ú·?\EDå°?ïÖãŒ+òÍ?l¢
¨{Ž?a¶Dîo%|?\ÆqYž?gf/¸•0?d£~òò?ïP"Z² s?"ƒùÔ(?b»'΂?wky†åÉ?"©±U'BÈ?'LÁé]Àê?î'Üæ—Æ}?–"|d¯ û?‹[¹ÚÄÁ—?‰ƒpÜbÌ;? C!Š5Æ?‡¦§ôü?ïB9¡iû$?~3ÔüÅ?g'—c©³›?U¼ü¶!¢+?"ƘêÂã?{–`ŠÊjèAGN4FGL J0358.7+7649?àuxþwu@1Å÷@=ݱÀ:ɬQ,B~À<¡ ÔƖ@c/p0?ýÑÍ¢µ¢?Êm®Ú˜A?Òc¢ýe?þÆIàô¡þ?ïv%5;¦¿éÔMdº¿â£˜@S,M¿Í5AU_ØÙ¿â-sk1§B¿ê:êýdo@¿á—}à€ˆÑAGNbcu3FGL J0359.7+7649WN B0351.8+7640?ïQhž¶G?‹çÀ"ì™?z~ú–
â?rö%"Ë‹—?Žf[p& ?†eñÀYôS?ë"lɁé¥?ºH>Õu4W?±j3¬ÁØ?±nöÕ¸Bw?±òf	؆?«ý'ÌÒªR?í¸¶ÁXá?›Ô
úi"?™U'q*‡
?'Oo6Áœ?§ÓàÛU.c?•|%_8‰?êÝ·[ ?—á˜&v
-?®+Ꚍ4Œ?ˆ'í$q?¹üOØk¢¢?'Ê0*ä1?íÛcWà‰?£ÛMy?–Jð3ò/d?xcO•?§$Rej¢g? ™!ºêì?æM±eW™?ÈSîΙ†?ĵùø©?Ä9Í"ªqP?Â"qœØò?¸Ý˜þ6?ì2'÷
…a?¢·Ú6í§ä?¥n"}èó?—!¨°Þ'?³Þ0ÿ'¡ø?œ}+\¡¬é?å³!ô'¯ƒ?«ìâ!4èq?¸ÝÐãÚEá? ¾ÂÆT0Û?Ìď¼v?¦•™ïOº›AGN4FGL J0358.9+6004?ﴅt.â'@°ºë#À9§)£gxµÀ;®êÏS)@X¥¨¼@}ïAkÛ?ÀG3å?ÄÒU7iù™@(
%ïû@Êú~5åë?ïõâlvK¿Ýˬ&w
¿êãÁ¦(U¿à‡‡émíC¿ïòÄBº³?îI"~Q¿AGNfsrq3FGL J0358.8+6002TXS 0354+599?ïÓ"jŸA`?láàEª£?W°ùW#cA?V±)U?p'Œx#F?f-ã'渨?ï
Òª:e?¡TÍå5*X?T,<\ô@
?aEýŽÙF?bæõ¯ÿh? çdrƒE¾?î>p}ìµ?–!-£¬a?Œ¢·ˆ>"?‡J2žÐʏ?¥Ow‡W?'vIÆ8,C?ïÊv'ÆåÏ?]óݯ?Påèa@?8@*a#ß?vÂë#±T[?ZD^Ÿ_»®?ïÁY¦ö‹?qÜêµTY?c,×	uÏW?azoR‹L¬?uåg¾w>ç?kl±%FÌp?íÿÝÑ?´ËQ¡»Û?i{†SîI?ƒÌ9çß?±("iq?´Wð®?ìÎ0:8Ê?¡'" dÎ?Çs"Šº?•i­kÿ?²KLP,ì‡?›l`øԗ»?ï>u¾óñ)?¿fºK¤D?p§\\uE?`?B×O?"qaë†?|^sv™ã4AGN4FGL J0359.0-3053¿í;`æÜÀHŒ¦ YŸÀ:ÖêedçÀ<«nñOc@ GʏÜ?ý¶¡è´?Ã,hÿ?³	ÊÀ>Z??ñ…Žd²1@@ó|ç‡8C¿ïþyzϪ?ïöþ~ö€$¿æ";ßT8ç¿Ó0êÄ.™¿á7u‰Ââ¿ØKéBNY)AGNbllNVSS J035856-305446?ïñŽßƍ?MìÎ&îq,?&$ºnô–b?<!Ìtä?Z©,÷»?L£ï$l£û?ï䋘$#¡?k4`€°€ò?2@7'³#?@ø²ü
¤{?i,a9+Fâ?hO9­¯}í?ï¦/¢'¬?r®%ÏÙ ?S
³+ Ë?9[!õ"ê?"Àõ·‰?rU4°B÷?ï¬ÍJm"?Wç!—ie?I3]ÒWPÖ?.†Ðq21?{ƒ-™X½š?VòfJï%?ï鵂G1\?YÝÚ÷<ùå?6>vbp?&ê)x›Q¶?c'®ë@Mt?Xð*ˆ1lÖ? ¶»¶?†õ˜,ûÌ?F<ÖÂC4§?UPk³?‡lJld÷?…ÚÑ~T%?ïhc¼=?{iÖ·??_ÇäʶBU?aý¬Ukfà?÷
#t˜;?y"\̶̮?ïgü7b\?tpoSrâ?[ÉÔök'?I£€rêפ?'bƒ&kö?stýyY/ŒAGN4FGL J0359.4-0236¿á·>"ØüÀCk=ÀTïFÀ;	3Ê1çÚÀ<gjÜì¬@!z²Us¥?úûÏÔ¿	–?Ñb{ö£ð?Éë~:R?üf\Ukl`@¡:ãUÐ?ïvé¡éÜ¿ïÿYM»?ïÿ¦=ìʙ¿ä|{±QFD¿Ãt0é×ʂ¿èèß½jY:AGNbcuNVSS J035923-023501?í¹~(¤äÑ?µó»eP¤¤?RfÇH4?GUæZàO?±ês O…?µô>i§v?ïc'Õ̔‡?'xØv&·u?m،ÇlÇD?xà;œ¿»?©'i=?‹Ì'…û˜?í¾72=·=?¢X‰&VlM?iÛɆp˜×?nä>Äd'?±?h"Ð¥Ï?¢"*ׁø?ì¼Ù¾^U?˜_ö•%Ó?\Ný`ŠÑ¢?PqT÷>=?¹§öª?˜;œXþ®M?ìAÎåçâ
?¶ë
Ž¢´d?f0+Â×¥¡?][eú[\?½@uë&?¶Ûò7¶Ú?î¢[4· H?¥\
x�t
ø¡"å1?‡;Lõ5¨'?£XížQÚÖ?¢2[þÍ;?ëú;hòîÜ?©ÊŒ
!Ýo?sŠSG|¹?z†ÆÐ ?¾õ"«²?©7<KB›?çÀˆÞáLa?±¼¿ŸÆº?f=Ûûbe<?f¡¦³$†z?ÐRr‰ñl%?±»üÏV¼fAGN4FGL J0359.4-2616¿ï"«.*ÆÀH>›A:À:¯8lÄNÀ<k5îÏV@"÷Ô7z@@J@Ejm\?ńüéõýs?¡ˆ6ð¬ûÌ?Ù¦:ý,)@++àÖð?ë:kkˆå¿ãó$Oj¡_¿å··6¿àŽ4á‰t¿Üõ¡'FA¿ïïуjƒAGNbll3FGL J0359.3-2612PKS 0357-264?޽åÿ?¦7TáöÙ?S³¯Š"·˜?x€uËÿ{?ˆ'[J?£é•|ËÐ?ï¤ín>2Q?'EݎtÐ?Xq¤ð&NŒ?]_§F'$?ƒ¶oÉ¥ÿ?tfª¿ä?ïdéêûó?}'2K½$Ý?eçÀ‡†Ôë?d×˪'?¥Ê˜¥9?z*D­Ê>?ï:ûüÔì?sJ¤[™û?aÚ¤¸QX?DÎy›}¼À?–"?"9]?rAê÷~R÷?ïT£Ai‰?ƒ§[hüVÊ?]泯˜ª?Pñƒ#'.x?",§<•>?'™Æù@Ν?ï$¶›],?–"[Ø?ˆ?bõ˜f÷W{?mj¸M>m=?™
yŒ¦™?"¼{'?îӋ»4žî?‹ðͨ¬ìd?rh¤9FÑØ?k~_×~? z/ÄYYå?‰Ô ºEòº?í°ýfÛÆ?‹ríæÖl?xöÖû=½??flϹ8ø?°èªk&~??Že\ÒÉ#AGN4FGL J0359.6+5057?í†2±O.¿ùqé¼ÇœÀ8$
!¼À;.•>Á@hDn
B@ÊâçÁE?§Hÿh^?¿×­?W@E™›@"Ÿe‹u¿Û­øᨦþ¿ãwµxó0å¿çlÜ×ÜËH¿éw>û¾R¿ìƓͧ¾¿ïÿ¸SåZAGNfsrqNRAO 150?Û8?'î¶[c)x?bL£ºäPÐ?_û64¡õ—?ƒÊž˜Oû?‹{†¤˜}?î[\ G'B?·{
ÿkè?Në,½¹Ãg?hô)ý¨µ?©Î‰I(É?·4«S6{?앳 †æÂ?§ü¤Fión?—¸KÜ-…?•ԅYÅ?µjøèѾŽ?¤qÂp?'™?ïÐ{¬ãg2?\:˜?!›?CÆg2 ¢r?1zŠ€@ó¾?uI\È1wf?Z˜ÌÿØá?îým'Üi€?—V·Ú'×4?píW§ËÒ?kø"[—?œLÒt47ô?•¬…7?ë?ì×"ëèF?ÁDmU¡zÂ?XÞP¡cÙ?m‡LóH@œ?¸æÃnlSÂ?Á?¼–ÒG"?ì†Ó/;Ä?§"÷DúÃÇ?›Ã°ç—h?•®X%W"À?´Øž—¼<	?¤=(?ê?ïyÔ:æl?zŸÕ?al\MŽ7?S À'À'?/Ú;´ÜÍ?yÎm(·AGN4FGL J0400.7+3920?ڗ̌­o\À$o"5ÒIäÀ:-idÒÀ;£J@·?ñ\¤@н¨"?ÉӎG€ó?ÓãùŒ|{?öWþ>^à`@&èãÙ®³?]ʶr¿Ó;Z^›@ä¿Õ9ÐfqN¿æ`MÈá¿êÔ­kÞul¿æ¹£Ÿ×Ì/AGNbcuGB6 J0400+3921?Ùi]Ïòy¸?Àý2)a¼ø?­6ª…%ùw?D$¿?áwæoFp
?ÁK"•M¦ô?ãÉY÷Üß®?Ç×fJë?¡—¾Ý|ƛ?Ë&?Ö:T5rŽÏ?Æ!í9€?år†Mó?²pPƒ|×?´&ßKI•?žd+×&öm?Ð;'¦†?°š ¥"J?ç L[xKÁ?¢'jYéj?³Ù¬‹-Î?ªÐMµÀl?ɑøK¼Ó? û{žÍY;?όh‡íŽ}?¾·ÒÃö~;?µåÕp˜ ?§|ZKSz ?å`+/È^m?Àì¶eñæ&?ٌ¡'ÑN?Êä®7WÒ?¯ùû¾ƒ²?²¶osÛbõ?á:z"¼W?Êî·&âÞ?Þó²=Ä™?´r\ŸÛV?¾Ì:!'?¤íƒƒ[(k?ÙY?A3|?³…ÌO|ԍ?ܱ­Y`?¬2HÐÉô?ÂåZFaR?£ŠYóæv?ÙÛ¥ƒÃՔ?°ªëA".'MIXED4FGL J0401.0-5353?ïÂdÊÁÀG*UC(s½À;NXø¿™ÞÀ<Ïq¾‰=@!í\MÞ°$?ùr_µj?ʏ˥†Í?°Io	Î
?晐?'Þ@ƒtük¡?ï×£ -²k¿äRW…øÒå¿âW˜" ;_¿ÖÐ5'BåÙ¿»F@V1dý¿Ó5½|!åAGNbcu3FGL J0401.0-53591RXS J040111.9-535456?ïÏ~
Þ B?uZð1šô?,ޕR×pf?$Såd˲?wZqÁpÉ?t·ôzE(o?ï´Òx)Õ?€Po&!R?QÐöRø?Z4j&Ï¡?€Â,"jâ?|*Ä"{úP?ï%G=^ä?‰KÑ!¶­?WžÔŸ‡¢Õ?C8{£Q$6?™ã‰Ï7Y?‰¬6+?ïmEÂú2ƒ?v<ˆ@³¨Ô?E©Þ\Šœ?1éREë'p?'©ÿoÊ]?v0N?;ÉÂ?ïª?œM('?)xQþØì?<uƒáë8?32¼ û"˜?"ŒlÈE͖?€ä¸ø>˄?ïY†0Üë?'¹…pt?Y[5nÃuj?f;õdö˜±?"9†‡¹µR?¥²ø'}ú?îS"ÇDD?—sɖÛzð?\ج'³q¶?RÃËr_èü?©ßî*ª?—Sí§ˆ¦Ÿ?î R'a?•›#¡3° ?\A¡›%ÌÍ?V©›ÅBê¶?­«íÍ+?•Çk2)Ó AGN4FGL J0401.3+0412¿è­'¥¸XÀA?Ú@RÖgÀ:>¥¸‹Í(À<
ïGK@7A"@±¤RZ@?Ãq·<íœ%?§cm1µQ?åujæ'è@y&
«ª"?ïÿµÂÅ¿éæ)«0ñ¿æq´]j>b¿àïÔ;V¿è°a&‹…¿ï÷¡Œ­"
AGNbcuMG1 J040119+0412?ï'ÙÖÔI?©eíû³¤?ag"}"Å?q»Sg­ü?˜áØ8=?§†·¼/Ë¿?ï‰ÂyÀ=ü?…,†Ò´Æ°?`ýŒß×(Œ?fV—áe—?‰OþQ~ö?ÚQk<Äî?îCnæ×SÓ?—ONTžSB?Qü…ÏÉ?yE¼Y‹W?§ç‡S¿òS?–fG "¹Ð?îâ¬ì»2?xË¢ô·}?pà@MG8}?P8/ti'?Ÿ":IÃfž?wOB*ð`$?îZŽ©«?¶8í. 2?qôOTÊZH?|ÎÞFˆ)Ï?¨‹†ï8?´òÎB;$?îÉ3Sz·'?›MÖ!µ1{?nê%˳?vxÉÄrsÚ?¡~(iŸŽ£?™+ഐ@?ëèä#«?§Rnðu3ä?–YÏ:v"¨?Ž¤_uzcE?»)
EÐ?¥‰ÍŠí_?íi4ÞY?"'Њn?ˆ= Vh•¶?p$î'BO²?´åLøp?"9-AXo@AGN4FGL J0401.7+2112¿Íñ-ÙpãÝÀ7?uÙ ð¦À9"a#0†±À<ä)à¤@ŽzÒ.5@G6¥®zÒ?±a¹ƒnßÝ?™";$³Ž?äêׯ~Þ,@9¤=Œ}|?¢0ž@¥ë¿ås´È¿çb P‡Ø¿ä¥U~Ž¿å°ÉaÕ¿á=u¬T‡AAGNfsrq3FGL J0401.4+2109TXS 0358+210?ï÷"y2à—?e°WÌq¿?!©2Ý{Չ?:p‡G~kã?MGΛçü ?by¼Ý~f?ïð¾ÉKZi?fÜÒ™?%Y²®‡?4Ü2æ3¢ö?[×7£G$Ò?e"M0µ¬?ïµ^"xRÖ?lî7à$ñ?UŸ²‹ü?@zÂHNJµ?€\1¼‹?k–bÖW›¸?ïó"ÈÊ3À?8m~¿íÑ? 7½òL?Ò"kÉ?VÑ|otO†?7` M½é?ïäȱàp?ƒ®	íÜhT?-j¡C0Hl?4uc@ôÚ©?i`£ËKa?ƒZˆA%?ïÌyeqžÔ?Te'º?>ù»ÿ[Pš?T"ôÛÜw¡?wÓ±gžyB?€±èŒA2?ï|lb(ê?}Ì®c:?`àƁ"¢?P4èÁ†'?Œß¯=õÍÛ?|n‹"l_Ú?ïÞ>¶ì?XW¯Ñ€Æþ?8*Þ{)ڊ?$9.oêÔi?n¼˜TÒ@?W+ºªÿAGN4FGL J0401.9-2034?Ç{Yι+ÀG3'äKoÀ9Žn™:Ï	À<]ʹÍÈ@UBø";@'<O;§v?¯Ïbpãm?¬© Øà?úð¥)œ±@1ûЛc?ïîíôdÁK¿â*^x[[¿ãµo¸õs¿ãa.A?e¿ê\w?&±p¿æ=¨6ëN˜AGNbcuPMN J0401-2034?ïí®ràq?]'¬!õX?3!è V@Ã?1ŀ覄…?_Ú¡BР?ZKüÿÙ¸B?ïëh÷˜Ü?g—ÉöÉ?0ìvì1 C?@Wm½Ú	?bÖB>Gõ?däò_çÇÔ?ïµE•5Ý?uQYx:#?bœŸÁz€ô?p¨T²¿?|.u¤?j¬»G4¹?ï÷ÆF\?25í	¸å?+Z"Xj?AbLRR?JDŠžè"?/¿ü§û€?ïÞë)т?f%ìò{m?DDJ'áë??ŠäûQ:?lÃU–¿?cŠPP"u×?ïÄß<³\?¿Ô\´D?=›\Í?QÖ*F¸?{¶«Ä-²¼?€¾Ebš/ë?ä•Z?€°þ§È¬?ksòaJÀ?uç}åJ}k?†¢Œ¹4µ?v·f]à?ïìñ榁?N5|IÍL?ADd$P«ž?0ðçfªÉÛ?_Wê<"Cæ?I³×]AGN4FGL J0402.0-2616¿ïþ¯9'Ç_ÀG׍÷¤ç«À:'C‹p+À<4–åŠ2ô@•§vQ?ÿëî€{»b?»§•/Ҁ–?ÅÒ.
ªRú@
«Ý3L]§@†Êk°??âk6¯Æ,?'‰ÇПÑR¿ßˋ¤cw¿á‡Öޞ†h¿ãxUFƒr¿ïûþ~ÀAGNbll3FGL J0402.1-2618PKS 0359-264?ïäŸà8B?d²ø¶Å¯c?U>Àѵ'?M½ ðp‹?`À¿êØ5?`%±ô9c?ï¶üÍ¡£?€Ÿb{ž?R¹À	R·?U‰#b*K"?Ӱԏ2?}^œbäÊ?ïI¢1²nl?Žo³çڌ?r©HýŒ• ?zÝÌ'¤t?'!gŒ^Ñ$?‹!¢ÓYLÛ?ïæŽ>ò"?s0Å"¹?k±½×+j{?NYvr?›löz$œ2?q'vRÌ9'?ïÇê‡È¶¾?y	cÆÚ?l»µN´§?k*}ìÁÇ?kYÂÚÖ³Õ?k ø|?ï.rù5¥B?•;…hêb%?e£&N^ù?p§é°^µ?—}<û¥»?"‹K …s¬?îɸ҈½?—w]ï^é?yœc/õ›?}‰x"Œf? :Ø
qÎ?–'"Åj?í{ãV¸.Á?ŽÒ'†g´?mºš?jŠ–G…ʸ?±ó.Åéc?Œ3½#?(AGN4FGL J0402.0+2737¿ï¦nýlZzÀ2¦•BCÀ;yD|	À<[Òç™í@¶†ƒ<`@`Ù¼ŸX?Ê(y›ÍP€?¡Ìud8#?ÚÛÏÊ@ÃŒÜÇÂ?îÏËOKE¿äùˆaãÊÀ¿é.f f¿å+§'i?‰ÄÔcw§4¿è…#ÀÏhˆAGNbcu87GB 035856.9+272842?ïs
óL'(?†äTööX?M8—š¦D–?Cž,-§­?´|ܺú"?†BPMŽL?­~B?•Û°5)'ü?crê‡AG?qœªÅaÛª?‹eKo{I?"VÄù<îþ?îóHü"\?ŒÐǃ6Ö¬?gžB
±»?hºÉ°Þ½º?ž¨dÞ]
K?Œ	m<Š?ïu_ë‹d?pça}
fÚ?;ÃQ¤'úx?+åB¿™'?äõQj¾?pºÔª‰z?î¥ë]Aà±?š	ÿá‹Æ~?cňJå?^›ïÅØä?¤dø7•µ¸?™rjº|Ô?ïV9GŸQ? \¸;ëõy?me)'%,6?}dV8=U˜?œ("¥—\[?G
•Ø?í—FÎÏ#??a©?u·Ÿ_ˆ"?q="µU,?±êO•n°›?œ½ÙóY‡?íëÎâ¡g?"/øÎÚÚ\?ZŸJiúÕR?S›œ¨3]?°7ÅÉö?"A
ÞÁœAGN4FGL J0402.1-3147?Õ&4¥ÀHEmã2iàÀ:OŠÞó­À<œ£Žåáq@nf½¤:Ý@D–eÖô?¸q¢"¤¿è¿‹è	û<²õ?Òm˜ŸH°@úþ½_Çf¿Êop»©äÀ¿åƒd£î‡¿æ=E¥ü~k¿àŽ1@¿¸½¿æä"pB]¿ïÿÿ" 5•AGNfsrq3FGL J0401.8-3144PKS 0400-319?ïí<|e´Ã?VIý?ªf¦??§rûrøÞ?4öeÙ÷«?]*¿dŽ?ScU`â"?ïà6T¶÷µ?p#Ïh¦=?9ä&»Þê?JÞ¡0Ì?l& Ó÷›?kva+ 8?ï"s3m.›?{	 б%?^ž$kÕn?eá‹ÀNúc?‡OnŸ'Nn?wqX ?ïäg¢ó×Ë?FæÈ-L/¬?Ioª|k%û?,©—O™µ?e<r:œÁg?Có¼ºUÝÊ?ïË(Ç?v'¹Íãð?S¯ÌÄ]m?G0ÁtSÉn?uxò{Ñ;?t~JË
Ãé?ï•4å1iý?ŽÛJj¼ŸI?Gô**4?XåÃèDq?‰3ƒÿÃ3
?æP]cÓý?ïûæ?ŽŸ@‡
Ÿ?l·8T	?pjŠa2ý?š'Z¿›	?‹É§E­ÿ?ï¹[0ÛȜ?eHx$aÉ?aP=°fÆþ?Mô¨Úz?zªH¿g®˜?aE»õÞÄ¿AGN4FGL J0402.9+6433¿í±¦k$^@!Ü¢˜E܃À;0uєÀ<Md;é»@!ë×ðÂJh?þZj)i…Ö?ݍ}K…:?¬1ž!'u?¯7Ö°ü6È@œ^;Ÿ"Y?ïûŽ¶çˆ:¿än­Aí
Z¿í~³íQ¿°@ô'âÁ¿Ï^z·¬)¿à¼-BXj$AGNbcuNVSS J040254+643509?äh+U¡Ð¨?ÊIµ¾ñËg?a[™*ÌB÷?]+‰>Ú:±?×ò"-º?ÊCGæ§?äj–ãB_?Ë—Ð|ì?ŽšA?5V?˜Z"⦞}?Ö6—Xv?Ê&öŠœŒÏ?êïð/þJs?¦ë'@×!?z¸ÂÁÀ†?w6"\TÄo?Ãjy)¦[c?¦–­"ç÷ø?î\ƒy¥;?S'·'wd?TeëñCd?E?Ey9??©"™V;?Ey®Æ?ÚB´K‡Îý?É%Ýԁw?j |Jöî?c•	pýÓ/?âĒ¹€"»?É,ÏάB`?ÚiH¬IÓ?ʐûä#ö?Œ[}‹8[P?šòj~¥P?âYí³»óz?Ê0=ÊæÙ?æÐsd?‰?°â—Á"Û?…d/Hz¿¥?''Oˆlã?ÓM=žN½±?°­ÈaV|Ñ?êeçGø<<?¬SSð/7?dí]ð¹x?ck–8r?Æ®ßb6è?¬sö=6MIXED4FGL J0403.3+2601¿"¨^ýœÀ3—®FÏÈ*À:uêe:íÀ<"Š•Ø@—ÿ-ól@D@¡±?Éò–J"³ƒ?ÑÕÍ\>Å8@ÐP_"äN@½¤ܘG?ïþÙY£	…¿ç®yZ^ñ'¿èǰބ°(¿äßS¢"j¿ïÿ÷!	:?áê8ÅCAGNfsrqOF 200?ïYýUx¨?ˆLßxöâ?s+Þ…ò?o SéRg?ê»¯Ÿé‹?"æ•xö?ïiú?š}i½R?"ffgDÓ?‡"§£1BÏ?•lɌ8x'?'¬Ò"3"‡?î/ß°n?—‹]/ŸÄ›?Ž>^ôýÏk?†K.E›g:?§mjFÝÄs?"G 2Ìò<?í÷}(äi?"䈛¾Ž¦?ŽâFÏ?nB'EõD?¨A%~©?-@KO?îs˜p=k?œf¦_ø$?‡µ84
ž…?…[TQ bŠ?¢Ù*ìý>¼?—[©ûºÁ ?í*®®…?µ)çb­Ó?¡'¯)Jh?©ÔÕ¢íš?­N-nÿæJ?ª¤§ã¶?ë'14DD?¦DBqŒÌ?¢†÷Ìÿ?"£'
Z»Ë?ºß²áìÎ?¢Ë¿Vx¤Û?éZ˜"²BÄ?£ýî{è?ª­Ë_!i*?kfԖ÷?Ãê,›¶Ì¨? "ñ›ç'DAGN4FGL J0403.5-2437?ãè ÍëZ×ÀG{SÞ¤e¥À:|%«‹3¥À<†:8
3@Fëˆúÿ@^®&˜}?¾x2–«'¶?"Úâ»x3?Ò)["æ^ï@

åÓYü¿ÛÖPē˜N¿ãòT{'W^¿ãn=Mh¿ét÷Ãñ[ø¿ï¼jÿR[?îÔ1°|4.AGNbll3FGL J0403.7-2442TXS 0401-248?ï÷2<¤\Q?EXüg?&
ÐqÂ? 
‹¦3R_?M¶
'àƒa?CӒ†!?ïÚ·]=·Š?qåk"½–?@gQXtÐ?MÕÞ2…¿?p—nŽ®z?n=½çµé?︔5y?qþ=F€A­?`€¦h¬^?jÁóè^?{už‡¨÷ú?h""gÉ'?ïì7³löÆ?F&9Y?69YÐØèþ? Úää÷ã?a!è@¬?DQÇc4?ïçJ7ÂË'?_¶oØE??æáðJû?8ŸU<<ï?d¹u*é?\µî+D»í?_›|?‰Úìß·—#?M§ñ¯…î?Zc[à̗?‹@Ã¹—€?ˆz¯þȸå?ï~ê9^	?ƒNôhR?lÑ[n¼ÿ?x\Ræ%¿$?‰vÑlöi?|4/¿ƒ¶ ?ïÊ9»sÅ?gޚHKäQ?P¬c@,C?G¸Ã''›?zÊYDš?exSó 	gAGN4FGL J0403.9-3605?àí¨_/:€ÀH=ÄڐïÀ7R}hájêÀ;¤eƒèWm@j/™@%Ø{V¸?'»˜¼'…?Áœa_–h@*9AÈ!la@!lð—'=2¿Í`ž—i¿âäZB@Â=¿èt¤Ò²À¿éj šª:Ò¿í@j‰
Ö¿èãD]}¿AGNFSRQ3FGL J0403.9-3604PKS 0402-362?ïm=™yÊX?_¤?v{ImW?väõ밎è?‰r˝H?ŠPþXD—?ïf5k>3å?›­Dʞïü?fÃ}Z%c?w¯)\õkS?`âð"õ¹?™PPb^"
?ì^0XÒÿ?«Î_‰íV?µyµÝùÄ?§Ï' ª?žSmÕï¬?šïÝ"NlF?ïòSõJšX?R	—¦ãþ?J³<µ°Ç?Fˆ¸=L?L—w'H'?BÄ.'H<?ïbÊá¡Vc?ŽìWÙ:+f?x›µ§èùë?vˆíˆÖ<?ŠÿlÏd–R?‰Ýë)Å{i?î¾Ã<f–?¬8D>å?uÅìÏô¹ï?‡AèéÊ?¡[nsmc?«(™éU©?ì{²©À·?«':œ?±Í(Ü%?¦eÜŒqe?¦Òî#H?¡¤?o>˜?ï×;è'`?jV½F®?a;'ÞŽæ?\g
ÉÍÚ
?gˆŠ~ü»Ï?a¼"*¤ÛJAGN4FGL J0404.1-1715¿î@¶²ÚÀFJ5çB™ÙÀ;CTxþŸÀ<Ì۔ìÝ@ )–ˈÿî?þïÙ\'HC?ËÅPV¯$?«—á€"‡?âTŸ^Õxm?ýQµ§—38?ïË$V ž¿ê‰G;þ³Ð¿Ï¨£¸+€¿áãÚÀ€c=¿ØÄúptb¿ä_@zAGNbcuPMN J0404-1718?ï´¾øØ]?xôn"…?:Ç%nP¡ø?12»¦Æ^?ú?>¸?xl\ê"³]?ï"fÒG
+?ƒ•iâ†mN?_ø—¡áØs?cW[ÐÆ	š?‡'8Š'd2?€M¼G­·]?ïX©n›5?)õ±mVã?d´Ì…"&?k&ÿÛYbá?'T8›ºÌ"?|?TÈéò,?E1/?xhjҞ†?_©tSG#?Fÿé%ל?œôñ%"¨?x/ˆð[?ïjÊ2W"æ?†µv˜-ué?J0Qdþ'?>À%qÕ:?'Õ73ÛÀ)?†?@)2JÍ?îèIýÿ{?Ÿ"l¾K(?kü*"¸2?vd٘•?Ÿ~HÐìP¨?œãîÑÁ?îÀ…¶ã¬b?š²C?·ÿ?h¥tL7Ñ?`'Æޟ&?¢vª9ü…_?Žomj~\?í
(U'6?"àɃL²?q•AºÇQ?aª(vÛmh?¶¦Z¡èñ¼?"èd7J	³AGN4FGL J0404.3-1559¿Ñÿ·ð
®IÀF
–_RuïÀ;O²——aÀ<ÁR¡ƒâ@Žèc¬!Ü@qL"îA'?Ô{Á!Gù>?Ó,Kb~û3?üBkK @$ñ[Í[=?ïëÁ¹É:?Ù-«ŸU›=¿åSç]DZZ¿×õ¡Ø,|¿ïÿúŒ—Ó¿è—Ý÷vÅAGNbcuPMN J0404-1559?ï¨Qéè͛?x³²t9î?h7K/!*?aq˜yÙÙ?ËïFe:P?s[ô'Çœ?ï–ÊA'+i?€™Ñ[?_Ô}:QVR?a^€}æ£?†RàA`é?zë>ÃUD?ï
¼'@Y·?i+Óé-?"4íúBF?"¨ØS®a?"-öÕ¬;Õ?†Ø+Õº¿×?ïOÆBÄ÷?p‡%ŠëaQ?wKËò
¤?\žW;I±?["GƒÀ?kƒC»ôfß?ï|UZ2??€pä"b®1?sËem'Ùª?h\lWa#Ó?‡åì#A]?{
ù˸ñ"?îèRÜ	Åj?œk¬«­?tël)†Ò'?…vÕh_Œn?ºÉo>4?•MMþ?î'ÓNÇ
p?–\O*BpS?‰)DYWQ?‰qü¬nÃ? ˆƒÅèo$?'^AÍ×n#?îI¡—B?Šî•N¥7Y?†HT£2"?v)o›‡?¥ÓÑh†ßÕ?ˆ¯…'NAGN4FGL J0405.6-1308?ŠšîÆÀEPíÍ9ÚÀ9wdå\æ‹À<KãýjúJ@oâ˜»ù@sÞÚŠ¬?ª»=RÏ¿ŠYE¢Ë?ÛÌӂÉs|@ƒæ2(œ¿Ùʦ¢¿¿äœ´&†'¿éz¡†Íå¿ä9Qàd)¿ïü'¶vI2?ï×i©âAGNfsrq3FGL J0405.5-1307PKS 0403-13?ïø;ÀËa¾?d2?:yß?.³sR«–?BnÐeY0S?Gdîi õ?_­°.ˆâé?ïê^(\óÿ?iÞ¨»wDB?3ûTÁ»Öa?Gh¿úð.?c"m,#ø?eªÑºœBq?ï²Ç|ùX?zùP£ôÎ?]{	q$þ»?fÐô	¶¼Ý?=Gtçë?xù.T§!B?ïúù¥×h?+'ÿ)ɸZ? [r'õ^?[Ò¨®?@§ñâƒU?''íò'äâ?ïó
½âèÝ?YÇÚFøTí?7wQ³Ÿÿ?6JÉÜói?T° Ék?W"˜'µ'ó?ï¹CP•La?"ýW*?@¼ól?S$̄§Àá?€£b9¾ü?ƒ%õ)V?ïq|'e(+?ˆEÙ!EªA?d[Ìqï™É?lÔ.U‡?Ž‰ì:kÚÆ?†Ó}í ê·?ïñ¯m'?L¸8"pw€?; k ?2"ÄÊ #Ù?UÜbz-?G0²$ÁãAGN4FGL J0406.0-5407?ïÒÞO3ÍkÀFȒ£"¯À:àŸd´µÀ<±2«M÷@«ó[VèÅ@¯àè@?Å
ÈÂ|?¤Õq¶ü€ï?à_o1CD@?ûH
ZÍ?ïæW¸M¹Ç¿êË
å›Ð«¿ÚƒÊE‰ø¿ãð'~Êá:¿éž%"ôÆç¿ïÿý±q&´AGNbcuSUMSS J040608-540445?ïÇ>$uL«?rѤ©'	?T-Nu®?V•IgÏàd?wU¨ÒìQp?qòàbûÖ?ïÀ׫Íùž?tùp`%]?IKcJ¢?P['C­2Œ?|j½©:kÍ?r™ò"Pp´?ïA4?ø"z?ƒyŽÄKòc?t‰@ôº?zX6>×´c?'·0°v8?|‡|×ÞÐ?ﲺ€«_?]–g†?`­G8à.œ?C6š9ΰ|?~Lþãq;?Y‡?L•‰?ïv¯¼ÆšY?†BÑ>N?i-¹šÂ˜Ô?bä–Af¥?Œ¢YêS²?"I',,j¬?ïIuÐø¼¦?
Zû7ê?ZJ¢ÕöHÊ?bªš4
?•,›º<C¬?ÔÞEƒ?î´îêâj!?wF|t?|èAEL5?}‰vz÷h:?¡	(Fò?‹¥_&f?ï/K¹€®€?yëu^òÄ?tbþ½f?`œ/ÖD?"ýÉU/BŸ?w÷Ѫ¤{AGN4FGL J0407.0-3826¿êáÖî(ÀGð:}ªOÊÀ8'pûëžIÀ;ÌÊ÷à@ÊÊÁ¯¸?@øfC*÷û?£w£%o·?¼¨ËæÙD@ÿE™›@Y؍Ë/>?èP«Hî†[¿ÝJŒL˜_¿åÏÞú÷­¿æ^ä&…¥Ç¿é!(n´¿ïþ'jöîßAGNfsrq3FGL J0407.1-3825PKS 0405-385?ïØ0	Kòá?e?»'Ó©"?Y¿Õägº?PªNàõ6?kFÄûb°?aíÄjÝ×?ïÓc"3Š,?xº¦‡þ6ˆ?H^Äÿ†?WDñ̋‰a?sKÊOÌ]?u·°_¬ù?(Äß?ˆ³ü¼í?i?·Ë¿Î»?w¢#¡‡ß?ƒÁÇâ–ª?"Ñûƒ™%?ïÛXf7[?T+ø%õî¾?M0T§x?:ŽÆʱÁè?m 'yÅ3ë?PbÁÒ÷?劣Ü|ö©?wk*Î9NJ?`ï)§P?T‹)ã¬ùÐ?'繐?tØ.ÊT·¼?ö?‰‹8´¥¯??W
"_8e?mû§ßzH?‡í´¶Æõ?†æ‰ÆĞK?ïrAôA/ö?ŠØ¢÷‡¤?qì_w$rÓ?zÀkR!ø†?ŠyS4!É?†ÎĒ¤Y|?ï¢ÊàÜW?qa¨% eø?b;
2U.?S@"œÖk?'¾š	ùúh?n¸¾6TÐAGN4FGL J0407.5+0741¿»÷¥œòÀ?$GäÀ9U¸éÀùZÀ;ëŽÑ¿zÕ@Ç=ûc84@Wn{ޝ°?°Øú''–ñ?£(:[ÆzM?òqV8ú@½Œqg÷5?î 'ódK¿Òý¼-î%¿æºUÑ쓿ä5ëß·‹¿âû"ÀĀο倴%6nAGNbll3FGL J0407.5+0740TXS 0404+075?ïíaª"é‡?T‹Ÿ°‡æ?+¤öHÒ^?èÛ
â?`í›N҂c?S—f,²?ïÜÃEË¢g?qKeÁ"L5?<'À.÷¨?H(4Òd?oª˜',É?n²Pó),E?!Å]Ô?~û,"‹÷?bgf'Óo?lþš¤Ú^?…?û}4??z6'ˆeV?ïŒnkÿ"°?c4?Q–w?d2@Ž¨?C#Ç6êèh?‡×Õ²^`?a•Iñ‡?ïÒ\°Òg¹?lÞ	€Ý?>°wŒrT?0xl]^"P?t謢Åó+?jÓO؎V¯?ï"Ë
f?‡5«ýîZ?Iz2—s ù?YFc¶«â?‰dj{?†±O¾?ïV<*E¾?ˆÎÓõî¬?e?CüÊç}?c·¯NJ²t?'—=sX?†ÀbKÈ­
?îÏ|׎i1?h1!u?|M>ü,õK?açYãò"f?žýSŸ?~èAá	]AGN4FGL J0409.4+3201?Ñ­¬¥SÐÑÀ,»"F™A…À:j«¾_KÀÀ<L)'ÉÁ€@ aùkç.Î@XKä ÷?»`¥_?¬¿n!¤H&é?Ö`½Z?ôÁ­]è?ìw~¼ž¿ééKRä©b¿àA|lb(ê¿Ó†_!£"¿à`¯"#¿æ'z-ǪAGNbcu3FGL J0409.4+3158NVSS J040928+320245?ï?wS†?Â*G?Q'áí#?G.Þé­­?‰½åﬢj?Zǖhø?ïf81¨?—OôlËp±?gÄüd»#¬?jé×ÿk¿›?@Nqœ?•ÓÄË$?ï;܈	Vô?ƒ½ãawö?iõmƒOÑ?hÂÔ§¿Ó'?•EÁNk'S?'AXà¢ßÂ?ìè/õnµ?‹tüClm:?Á›r5Z?mQXTá?´ÆLçš‹?Š	¦òȉò?îíã͑» ?"èQÒÝ®?i:<"p2²?bAÇûø£†?Ÿ>Ãíҗ?'Ô-­vì?îmËÙn!?«²Œ¨Çb?zä<0Gô?ƒDâ9ÈÜÿ?¥ÆÂ`|y?©ï‡°	³ã?îw3½FÈ?'Mþ}®]t?t˜ÔÙPà¸?p{Ò|@Æ?¥û"'u¤m?'èÃR™­?çþÄ5pò~?¢÷L­K¶?¤Å
¿)S¿?‰©Ÿš;_e?ÊÓ¬zqá?¢Ö©;ðhAGN4FGL J0409.8-0359?܌"Ž'ÞÀB°€Ç:¼"À:0î'hÀ<K.cÀ™¹@¯'aÁæë?úօ˜ZÕ9?ºê!Fv²?ÓÛgšC
@ý+¿¡k@ö0툯?ï—ÆZÂÄ5¿Öµžþ'U¿Ë"Îš¿ßW
:M"¿ç6Ë£×àý¿ì+½óëõ‡AGNbll3FGL J0409.8-0358NVSS J040946-040003?ï³Å˜É<?Œ0Ùf¹—?l`
ïw2?z¶!Ÿ?wí&ZÆî¼?€Sîx]?ï¿Z[ɲð?ƒæèvˆ]?PužŠ¬?Xàðéâ/S?|5j–†õ"?zâOÏKÜ:?ì>Áê?ªaÌ! ú?²Ú«8¦°F?¤7<‰'Æ?©)e¥²gØ?¦WýsÜç?ï+~ól?q$›±ç?jCþ¸Ù¤?JÎs;ôf?—GÀŽG?o´N
Ç?ïŒMeZð?"êöXŒ^?z"G‰F²6?wHۋãjÌ?·«¹ð?y<íµ'Uþ?ï"G×@Tj?¤Yâô|JF?s2WVƒ8g?˜½G@'Ú²?–êoF 'œ?–SáaUñ©?ê¿}¨«?­^Žµø»a?¸ÏVÑN?¨JÞåƒ÷?±v·îù…X? ã´©l)Ý?î/ˆ€º?Œþ'2Ea?v¯ÉŠæ¶ø?bŽùæò!?ª1…ª–šu?Š°¦äKg´AGN4FGL J0410.9+4216?ê·f»ÎÀ&Üã›EÀ9t»=¤¦À;é?l&š@vI±ú¹o@ËN˜‡œ?¶®#ÿ¹‰#?½ÞúaZë@î"þ"?@X1` (Õ?ïµK;gµ¿Ÿ¤,€Í¬¿â<à<Z¿âÊ|ûÔ!U¿â¥É㽿맾ŠßÂAGNbcuB3 0407+421?ïÏ2Ù­A'?b'»Ùñ?<,;e?0¾L\‹?v£ÏŒ÷s	?aG5ƒÐ?î¾arr±?¤ÔŽî2¿?P…ä‰#'?`¬ó>¬³/?£•À§<©Û?¤`ÏÅùU?ïJâ½W—t?² £éq¦?i#̔ø*?dçgF¤îÑ?".ÀOx?oàyN4?ïU3RŠ2ì?lñÑ%cr.?qC&›¢>Î?NšÅ(äÖ÷?'ÌuËß?kpZê]?|Ä?vYŸ8«÷L?OûTJ¶+Ó?A=ÉèµI?…à)b÷\?uL­ÉÑ?ì]8ÏC8~?»Ûàë+¡]?`ÇÀ'á?p}3'ŽÖ?¼–Hø0B?»Šß'ÔkŽ?î»Ú?bQÀ?'#üT;ûá?wê3ë?x\µH…Ú'?¡P>¿ó…?Ž0
3ˆ)?îH'ˆlåJ?‡Zs¾éŠH?†Yþ7ίm?k점M|u?¥àgìæ}?…Ö@þrÃ3AGN4FGL J0411.7+3041¿ëöÇ{Ã߂À-ó—»s5À:ÃÑðøüÀ<#AՍe¯@mqÕ‹@pÈ¥ߙ?օÞzt:?慍Þzt@oçáüú?þä#›e¡š?ïäÊ"%¼?´'ÿ¡‹U‰¿áˆÞ@<±¿éÆh¸P>¿ïÿ}#AM¨?ïû?!ÎAGNbcuGB6 J0411+3040?íû€…æ"M?ª/Òºb-?¢6Qð"{m?£Íº)ò?œ#Kj©Åu?˜â<@e/a?ë1D4|"?Å}ÿ_F6›?µÙz"?º¨¶‹‹ê?²LœÒ{eç?¼ÁëOøC?è¿[^FH?®¬E"oõB?¸zãÏ\o?¤òâmð_?ÀøÕmE(?¥‰û|Cº˜?à7éQxÿ¬?¯†6ÕZ?Ï!0ö±¼j?¦ôÓXÛx?Ïÿ)ÃjDå?­Pšl²?ënN#m…?¹DW»nN¿?¸>äÃØ­?´Eß<2"?¨TG׏[?¥QTäçSi?âp^/òGA?рc隟?Ѻ{Ël>[?Ïր?U€e?Âɏ©^fE?ÃAÝ&W?å"ïs?è£?³•èŽ??Á©@éݲV?®¥?!ûi?ÈCI"«?­|‹–±?Åvµ>Û?¦V):2—1?ØàøÓ?¹¼Œ«Ó
²?Üdžhhý£?¹Ë9yÉD­MIXED4FGL J0412.3+0239?àŸv…mg·À@™3]$žEÀ:4±‰zg¥À<³˜H`Â@r_˜ìË@b%#¥÷v?ÁZÌ)cь?®@Ÿb4?î"ЧLàƒ@3U#‡¿ã¿9+
Ë?Òµ)­xs¯¿äâ~—_®¿ã Þ҈Îp¿êŠDý`¿Þy–ÄÓHAGNbcuPKS 0409+025?ï‡j!Üɚ?ˆë¨0ëm?fµÄ&›Ú@?~Ç\«ú6?ˆxŽôÖÕ?€IÉ7«6?ïÌ Ðª+?tp͇"±'?C+ì!˜Š:?J'熆|?wŠœU?rJda°G|?ïA\ö>úÖ?†|olhkÌ?rhMÎrÃ?tde("†Ü?":MîEN†?'ŸÖpÖò?ïdœ%§Q?dÌÔ~LÚ?i¢y˜A‡¹?GKb"Òˆ´?8-zã?b"·—djÎ?îàèflÅ?"qլ˷?y1he?pBëQ8'?'·ÀP?'€æýL2?ïZšöÕ¤?‹Åԋº?W"»þ঍?bÞóÎíÜ?"K èBt?‰Øw|˜"Ò?îPj$ÿ?—ëk²üM5?ƒÙÁçl'?)Ìãa$?¦îB¤{†?"§î@G?î}®Ã¸A?€¨-½qÊÑ?Hì±W?dëÿ6—o?¤;ö5²Ü?}‡š–AGN4FGL J0413.1-5332?ݔЃÝçõÀF\Ïkã}éÀ:‹…ÛÀ<QäJ—ÓÇ@±Šû"@/«SÖ@ê?µ¨Á?O÷?—°þ‡|X
?á`fQÒ@Ußêáµ½?ïÒéçÆ²¿âIfÿQ"¿çVSÉ«°¿åH¦4¿è|z¤áÌ¿Ý·Oµò–AGNfsrq3FGL J0413.6-5334PMN J0413-5332?ïõŽ®~¥?GÐ3È°?yf¿Í ½?
Ђ×C?S2 ·Q?FŸ1×òÜ:?ïïÁ­Îž£?d—ôŒ²?%6îW/¸?8'ÊOËk?]ÕƸ
ð?bzÎԗ"?ﻎó'"F?h½È8­«?Tc\ó¤?SÕޚãÉ?}¢DQ€^?e¦'D.,Š?ïúl³¨?('+uAîw?–+ú>÷A+ÜE }?D:oPûÇ?'¥‡Ör9
?ïì•ÓDÝ?W½ âF²E?*MŠöf ?˜òµÎÖx?aÅT>Ý¸?VÝ\ŠÅd?ïÊì!¦Ä?‹7æ} ]?:åYòÄA?Q?þ @?yK4]áüÅ?}˜šs¼ÃÉ?_¢?|˜r…_!7?a-Ï晑á?azݐBC¤?‰ÈH2è˜W?yB,ŽÁê?ïñµRÞ?Gö³L'«û?'ú#ÝXú? =¾ßxÇ?ZÁQ[ù¹2?F³°I¯–)AGN4FGL J0414.6-0842?æς^¿~ÀCW¼]éÀ#À;W‹àsr¾À<§ü­e(y@àoW%Ö©@æ—b%?Ç鮄ã)0¿…/n=Üj¶?¿a@Œ¸	Ç@›2֖û?î©z¸-˜¿í;ž§"?'n6'ž¿æ¼ˆabñg¿âÙA…Þ¿ÔíUBý€ŸAGNbcu3FGL J0414.9-0840NVSS J041433-084206?ï¬<†öÄ?'zÊƕ*?9º÷†ƒ»M?2i¨Æ/þ?"#&lƒÏ?Ê±›ÄCH?ïº\•,L?y#–1¨?P {|Û?Ußñ>©ƒ?~ɖ¨HÂ?uGîÕ­ëd?ï¼Óãõç?{ûž®µ?^Dzbé†M?[+kvm0	?››êa<»?7'o\6ë?ï¨ÉLå‹à?aløµ3­?@[ª§Rr?*ùGl¯ÝŸ?"Ä·Ö±ú?aC#–Š&ÿ?ïœg÷'?˜)ídFüi?KšËø$?@uþêø?œá›ê@uó?—ø|똯?ïGÈ¥Šç?ðÏþˆñ&?Z'"W¾jx?eѓþž"Ò?•]Â^߃?ŽæÚ«aâ?î6…zÓ°Â?—­™¡iV7?eïZØö÷"?gèötù±?«8²©)n?—výžœ?îí'¹`?ƒyܓªô`?Tp¤ñ")é?Iéÿ}9aý? ‰ÿDY¦X?ƒœß½æýAGN4FGL J0414.8-5338?ßñ»"o/}ÀF9Ç͉‹/À:ß´tç2ªÀ<ŒZ{v™@!Æ.Ü"?ú¿$º|?Él;½pc?Âu	ÂK"~?÷Dî|Iýz@¾ØR'ó2?îQí}ÇV?×/!°ÿ½¿ÃW—ULj¿Õ]ä·¥¿Â®9#b/Ë¿èg²GcAGNbcuRBS 0526?ï¥Äƒ¹C¿?{IÔ+ù?FëÌ:ýŒh?9˜j
Q20?… "J²Ê¦?zŽ<òŽMA?﫧Y†ë'?ߧè3R	?SEî<â?Xä½M)´?'­ˆXêœ?|ƒÁ_óé?ï;ˆ8?†&"³ŠZ?[¼ÇSã˜E?`ŸïȝÃ?–Ó2'֙æ?…ï?ωüª?µhØ?'¤ZoŒ$?lóIÔ?UrÅÿ¯÷J?¤7RË«™ß?'‡)ɨ?ï%m:$ª?Ûxfbt?`\sf³¢?S'²ïKgà?™FÊL'iz?Š>¥Æ^?ï7?F£?'€L/z?aÆø†?gZîí—Ë?–ã?¼Ó-?ô
)\?îgVŠjŒ?•´NV°Ù?b•3ù«¢?e/oâl˜n?¨aF)Рü?•n< ›‹?ìPuC_7?ž:Óus+?'ó$¦Y?qñgæ?»ŽL&§½&?÷ÎèŒÅAGN4FGL J0415.2-5741¿ÙošÑ–ÏÕÀEŸaܓê-À<1 'EÀÀ=Gýœ@#`ãÍDkë?¤=Æ_u;?ä':l˜•?ïüšò?ÿÛÄ?þ©úE+¿ïþæ?d™Þ?î¹NjÇ7¿Ë©nù²Þå¿ç8Ð@Ô?¤0Q<Ľ›?Å¿ˆÁ…AGNbcu1RXS J041505.7-574237?îj2sÃ?¶wÂúf
%?t$¢sHQF?v)ñ<V?¦ØKL'Û)?¶XÂPÊA?ïG‡ËæÈÌ?£ÛJ;}þŠ?n`òísˆ?ºïGÅ?"Bè+#Ï{?¢–úM¦‹?ìF/?ÄÍ5?©úÃ7õ%6?¢Á¢9_Îñ?šJ3©ƒ?´m´æá|Û?¥€pƒÄÇÐ?뀋ï§?®ý·Ã~¯?TaëÌ?Ua'Ïo=Ì?Ã]<í¾p?®÷i=N8?îVU
ðÐÚ?ªÖ'^Áö=?ˆJé]Q>â?ŽP&Œpa?¤‡ôÅS¦?¦ë²ég[[?îùß÷Ä??·'–;³bØ?‹Væf‡ç?¨&C ;3Þ?§OLE2L?­'d.^±?ë˜d$í ,?­7*ÉEj?¥/Æ'?ŸÈ´Á¡¦?¸¥TX÷ÜÔ?§¹p2CÔS?çF¹Lè;?ÁKEù‰nS?M]ß}§ž?dŒð¹õn?ÑèÄBõ?ÁR؎ÀÇAGN4FGL J0416.0-4743¿ï´|è3IÀF½#N¹¡wÀ;fÞõÄ<ÛÀ<ßùË2˜Ú@Nšþsì@xä$Ø&?Ò-úNw\?Ë!É(}w¥?ø[Ƶ[—@(¦h´õ@?ïù–Ys8ݿތ¨ðN²¿ç›Ê`áÂ'¿á±§­Y¿ïÿ¯Èe_¿ëý€Ú†AGNbcuPMN J0415-4737?ïݙM:è¬?`©Sš²å?Rg냿?FW¤tU,^?iYþ‹ýø?Yã€kÝ?ïœ,\"?€ÝŽ}Üý?_‹Î4•Û·?cXWÖ½ÓÁ?…o3/%‰?zð'MÈÉ?ïF˝$¶?Š*v²J%Ï?s®½%c‰Œ?v̼è›bÜ?':ïÅ>EÝ?†^ê'?ï«œ´Îv?`5Šÿ"—?bâý¤ÿ©?EœU‰ 4?€ºàDÚ¼?[ÁÆ@7î?ï°çöÁ4`?vi[j?bRHœXë?U3ƒàÖ·5?~bàIª6«?sýŒ#äˆ?îø¬ùaš?šÅr=ô¨?oô˜7€µ?{Á–½6!?œëÍÃí«?–˜›;´?îǯX ‰?'Ýì|6ÿ"?}øõ=¼ö?€C­'	³v?Ÿ‹à‰È4D?ª_µSP¸?ïí$±W?²vÁôž?ub±ï‡}?d'ù_M}—?™þ'ºJD?{ýH$áõAGN4FGL J0416.0-6628¿ëœãˆÚÀCí½Q.ƽÀ;C¤as¸À<»ŸÖÊ|@òs\æ`@Gý'w>%?Â;…èí¿«£~€Ž†?ëIA'¼Á@º•'LC%?ï–T€4éñ¢Íõ¿硑J?¿3¿Ý½"ÅÌþK¿â&¦'¦`Q¿Ô´AGNbcuPMN J0416-6629?ïÀƒm)Æo?­S©á•z´?o<~Ltj?­f#¬é"?p ;:dê?igÓ&ÄÂ?"@a?À.®g$³?_¢²H?bU›?‡#¼F–Ì?}¦®l¾?ïfïðæ ?{lÜb•A?eözå¤0?oåk.Ã&!?cMB®f?vZ?¯%j?ï""~2Ç?l¸HÜ<×?S:Û8'e?:tˍ³"?ˆ–ÿ½8Oë?k›r™û?襁Í\Ò?xÅ<""©?V	L¥a"?O9óÛP\?''*$å¿A?vü	]Nx?ï	7Ô$&r?"å~Œ‡i??e
_QÕÑ?l›iFx[ó?œ7Sp˜Øú?"!õ/gX?îáÍWŒ-ö?‰Ø`	ó!_?q­y'º«K?vAÛ¯£"?ŸZöËÂÄ]?†è‹rÁ<?îb^sA¯ç?x$!Ð?rà‡Q9ü?a㶂ºXL?§~ÞØiÃ?¦q±ßfAGN4FGL J0416.2-4353¿âď&ÜÀFðîcŠ	À:ßÇÏ7
XÀ<žÑ0ߛÜ@rØòõÖ[@Ð<eáÜ)?ÆH3
‡¶?¿pQ¡³C?óÖރ®uÊ@a"²VÔοïÿÃ.¾Ym?ïþ­ŸàÛx¿æQìAZ¿ë3^ ò"Ü¿ç"¢^º¡¿ïÿס<%JAGNfsrq3FGL J0415.7-4351SUMSS J041613-435057?ïø@.¯?gAüÅÿü??4êŸÞ½£?fAN;è³?E
®¸xJ?=G·Ô,Á?ïã[v:?lr7-%kŒ?8]ñ]Øÿ?FUÍÜ®?i˜Ëã¿)?hÒ¯ì+?ïis·çÑ?‡·g¢àññ?p¾qƒe¦©?zË:;"; ?CنŠq?ƒƒ}Ö?ïæf1?ñ?HØëö©i?Dm[¨&‹?,"F·+?d~w³'"?F@">	ùë?ïðÒØvñp?TOb\Ï5s?:q¹%6ãL?5øfíŽËB?W½àŽ‰9â?R˜R>Š®?ïŒH"—îŽ?'Z]!KÝ­?Sf]|'ÜÆ?m 3ø?Š(
g
?Ž\xC6G?ï×ép?'	½s1ˆ¶?xk"—¾?r¦4åil?˜<HÝI?˜Šú—?ïÀ:Æጉ?fs™6¤'?W§î¯•@Y?H57]w?yø ï³‰?cè@V÷éAGN4FGL J0416.5-1852?è'ù2öWÀE3§Å¬À9wc(ÄDhÀ<[²h!@†Ì<Ùû	@ö Ä0F?«ˆ>®ïö?¢ä,å¼1õ?óõãFŒ@Ge€¸L7?Ã_چç¿ãuÒêóÿ¿æ"	\ ¿æ'ä¾®&¿â‡vfœí¿åm¹ Èw~AGNfsrq3FGL J0416.6-1850PKS 0414-189?ïõðBÙՅ?O2Žeù?—$™üŒ?ºùdˬ?Rf'ŽÂ	?MßãšP'?ïïwÔÓ?d"_û†}?'9òF$õ?:´ø
>*d?^ÛÒlՆ|?aÉ_Ñí/?ï´¤ƒ=ÈÊ?uI ‹b¸?S*1T%d?T'¼!—Ì?€q™_×?tœùdI
?ïü¢HÐåq?­ŠŽá®½?Y×F-—'>øJ×¹(?6×D#ÀD?Òª˜€¦?ïåp"ö?p-¡Ð'&?+ÒĨVγ?.ÊÞ҈"?i;cP*éy?oÞã1áw?ïÈxíw4?~3Ě"§\?8ýæ5!ï½?K6%n<é?z4¨Õ&Y?|¥V.<€È?ïv-Æ·µ?"R2éÀ…7?]$´Õ?U[Ž?ŽÎË<?ƒßý68)Ÿ?ï÷é÷]¢¦?=çéšÕ5?$¶¾ñmàƒ?êž,Í?K*s;
o?;4Ü	–#AGN4FGL J0416.9+0105¿ït—Ò<èÀ@"¢ƒM&úÀ9¦¾r–öQÀ<	¹07Ö0@ rÞÎ,j?þ4rHø"?±en™»¨b¿†:A"ÖJ?×]_A. @		l¥Å¡à¿ÛüÑö®H¿ä¸u\£o¿âkIYæ%c¿Õ՞Bà¿áÔM"ÞHö¿Ë¢‰pîUAGNbll3FGL J0416.8+01041ES 0414+009?ïóé¹äà?KþÙ¦?$Þ¨à^EB?û"sç#?VDW«ŠU?Há·c÷5?ïÞ"ÍÁƒ?r3Ö·®?5-øfþ™¨?AïJ~¶d?nÚ¬ô"5Ý?pê%!öhˆ?u¢™s?}uٕñåÿ?QÞjG1Bô?<pΧ
fi?…ÖUF4k?}`9l§z?ïmú]9þ?næfRL¯'?P&qòØw?3‡c'Tb?'>S·÷í?möú#bq?ïåÁTÀîê?_6?WÝÐ>?91R›Õ§"?-²àË}?g€®ÖâŽ?\ÉüÀ´Ö?t•?‹Pn"Æ?J¶±=)˜?Y—ÞF?ŒZI>æ¯G?ŠÌìÅã?ïJ|"¬ù%?†9Hå»Êá?[ YdêÍ?Qw©RFæC?"ÿC'æç?…ýcW8,4?îsNí+š–?‹›è	†iü?fÈQpQ[?R°etŒ6Š?§^Œ=?ŠèŽ€m¢AGN4FGL J0418.1-0252?Ò¥†Þg:2ÀA…
¢q›À9Áíûñ}†À;ùôñ¯e@FÔ¸~Œ"@(N?þó'?¹5T`)‹j?ÈOFúTv@
d8Š‹	@™—‹wlô?ïÿ >ybm¿á¥ø¸
"'¿ãm9ßtÅ$¿ãéíÚcŽE¿ìo>±ìv¶¿ïþ–]úÝAGNbcu3FGL J0418.0-0251PKS B0415-029?ï¬}¹œÍ?Z$lNd?kSÉhgZ?c¡aÉ"$?|LܯmÀ?Œ2é»?ïáÅä•M?pN½RvŽ?;g‡ÅI?K="£¥­G?jÙN¤I"'?kÍ+±z‡?G·?™y8;Šäƒ?—¯gÔb‰?"`l†£ä?–Ù8¶—æ˜?ŽÏÆ>iý?ïÁ R¹õ?XÿvÇ¢`|?L°›²$'r?2>½Ÿ«¼?{™ÃxvÇz?V×Ó1mD?ïˆa^s‡?"±ùD¡…ü?w•:	÷/¹?s±˜Yʆ?'¥öa?|Uf½7ÿ,?ï¡oþâëê?…yÇp?TdmÆ·žå?n
íE)S?…r"Ï)–?'ᘔiŒ"?풹"¹?¢+ßÜèÜt?¥qZ+ÎW?›V×'C»Â?¡c–GÒ?"‹_Ö:ší?ïaôBBÖÐ?v3OV.%?aÛ?H?Nì挷µ?'†ı.è?t¢M™ºÆAGN4FGL J0418.2+3807¿ÉL,È,vÀ!ˆr)é–À8ôÅÕaÆÄÀ;mW…!@þ®ð}@ä_á'p?µæÈÌbÏ?Ã11{M(R@SƒãNïQ@
j‡ðú©¿Ó7ØßT¹Á¿äÒ3ß*b¿é¡ÝÀý¿è>°	G§^¿ëØÔ½‡	Ÿ¿ïüøÿZ¾'AGNrdg3FGL J0418.5+3813c3C 111?ïqìçJì?†"or¤nQ?f@hn2‰?b¦1¤? ?ô¾[Úl)?ƒ"ïCá†?î(S´e«^?®T«–%¦?b`_v™K?ofcL»?¬TÄd‰Çˆ?­'$¢n ç?îò#rî+?""a€¶d?8=ÛA(?…ÌÜU?˜ôõŒ"ߌ?ŽÍêGö¨'?îò$¨´rA?9 š¤ç?wå5Íø?X!yuUxH?›Â'Ø67u?|•Ÿjè þ?îSûÑáÎU?¢2׍'ûl?wˆƒMN%Ì?uÕá=†?§Ï2uћò? àCÑTàœ?ë!2£§u¶?Â;­S<?vàH{Ù
"?'®`ȼÂ?ÂÄ3- kþ?Á×0ËF\R?îXC½2ê¨?	~ۇ™? g€%?Tc$U?£3ªd]›¾?–¾¯gø?ífjÈuÐ?—ÄÆÏúØ
?Ì$s×Ý?{ÛdR'‰?°™¡òX¢ƒ?•aFîAGN4FGL J0418.4+3414?ß¿"¢ÎemÀ&õû"‰µ À:¶XÆj²üÀ<-+œeü´@¥4°¶Áž@yõÅšç?Ò»ua€ùe?Ê¡õHAe?ö	Œ³?ó9
}‡jB¿Ã>ü•t¿íà
¹(*¿´ZŽýðlu¿àÚ&½+.¿ïÿÜßi‡ƒ?å;
óÊAGNbcu3FGL J0418.2+3412GB6 J0418+3411?Ʞ—‰š?¿¥¨Æˆ:!?"Ñ=Ŕg?"oäƒ;£?Ãc{"9Í?½÷,Øâ@
?ê1°SðB?Á¾"DBr?‡"Ôei?Ž€6¡î?ÅÈÖaå¼ø?Á"jx™Ä¸?쮙k©úÃ?£,0cäŬ?œ"¨üµ‰?'<©Ñ
¤=?³ŠOz(ʀ?ž¿`n!=?ë?Ù@ÅåI? äõ(.Ê?7Æû-†—?t&õ˜Œ?Àù¢8߉?ž² Å?æרîh?È^"÷mi? xK춌?ŸY|Wµ?ÑéG0/ ?Çù¯—:wS?ãÕÓtíÎá?ÎXä)­ö?—¯‡fOF?¢'R$@û>?ÖÙ`¥B€i?Íå9d>‡¿?én€&^—?¯*Ӟe?Ò?¦Ã~R=?™¼F7‰é?ÄÀ7õÝÒ?¬Š -a«ú?å˜UÈo¬?±Ï]½‹Á^?—X\ê:µ?‡A_w³
œ?ÓYΠêú=?±UODþ AGN4FGL J0420.0+0805¿î)ǁ*ÚAÀ<sz€Ïž8À:¬[y£Z
À<e|[›1@‹¨ÉR9@rT`ªdÃ?Å}
—³f¿"9r½aÊË?Ê·û–ã\@
Ðδ®rð¿ÝN'}ÁKå¿ã:}¿ÉY%¿ëˆ:̄¨q¿áåuoî¥e¿âàØóK½¿ïÿùµc#¼AGNbcuPMN J0419+0804?ïöˬøWP?F‹üåþ¨æ?'í–MË?¡YZÜÆ¥?OQÃs?D»ý[I9
?ïԒ²…ßå?‡0ˆ¿_n?:~«P]ê¹?Dh¬•V­q?t¼DW¸?†'7~ü;?ïnÁ›¸¥?…?À¾¿<?`d…±ù?avC. j?Iýï©?"¡ª~†?ïȅh<Ýß?X¸M&_ùW?-Õ[§iàÂ?7uQÃÂD?zΡ
>®Ð?X@Ûôÿ7*?ïígØ4³?[l"vFÝ¥?60ýùã¥?-žOWŸWØ?_©ÃÓ<õ?Yƒé')«?ïe&î+l??¢·éÄ\ïM?N䱌ÖÅÑ?^ô»ú§±v?'cü©´Cê?¢'ªë€¶?îߛ;㹁?'ì²ôží?l·!¬-‰?m?`KòØ1? :Ú%Èã?'68¦X¨?ïS¼À¸"?z¦œ‹V?Go.ÿeÍg?6®Ý¶]ô½?"Ìîƒ÷]ÿ?y±–ôwXvAGN4FGL J0420.2+4012¿ï™iqøY²Àf'ëØ+À:=k¥jˆ4À<q¾‰=+@!	'Oæ?ýHÊ#¥ ¶?ÃwA)@?¸NÇ~¹ï?ôòôcê‹$@ÒÛðX•?ïë³ýÈî¿ç Çä¡Ö?Ípž"ÀI¿ÞÔna‡"n¿Ú] #÷V
¿à‰äð°AGNbllB3 0416+400?ìÓ
fL?®†èýAû?`îÇZ´aà?L‹àfÍÈ?¸à'ïÏ?®qŽ;}E?æšáQWû-?¿¬ép­£?r£ÿüa?uI7{+¿?Ò±UøÚó?¿töeç)^?íJFK؊_?¡hJ5;?xÿØM›?n:BM¯Äª?´,­£ŠàÎ?œãWô4Ä?ìzkþ€Ï?'EÜ!6X?zÑûˆ£?a‰ _Sö?º'lèqÕ?úM1¸¿?çDïY-ˆ?Á#Cb;›?v0¯$ç/@?göœŠªà^?Ñ	dF•T?ÁÐB"9?ܒò‹xC´?ÃÝ{™‡Ç?uD]ÉÿþÖ?†ôvX"¶ ?á‹ýþâ¸`?ÃÄcM=†¯?èjܾ÷?°€]±>¯q?‰òÄU?}3 B;Q?ÌÄ-â€×?°
÷æíK?çQ@á‹d'?§ÚmQñ?ŠÞ´^©Ê?zqèûٌ?Іþ…×p?¦Àzö>«ÏMIXED4FGL J0420.3-6016?à$—óëäYÀDäÁ¨¬\À:ï¨NhBßÀ<Ҝ¡‹Öb@ãü>Ty@Stÿ†]}?ÀíS*Œˆ¿ŸWÐýD0?ޜš·På@¬ƒ!Ýö@?ïÇËLp¿åvÀ4ü¿å¤)	ä…P¿×",<žìÀ¿Ý@IQë¿á¸I©ƒòAGNbll3FGL J0420.4-60131RXS J042012.8-601446?ïÛ»
¾±?ˆŽP£'Ì?C‹B7`Ö?_`†zpp?ob$ÛR0Ú?…?£Ó*t?ï×÷Š‡û.?m¨Uï'Å?9*?94 ?C§"?ºŠ?rq–Æ''5?k04ì"êè?ï¤MEòÂD?n~}½ÿ­/?UU0¡I?AÁjŒò€?"Bo,Œ?lߣ¬&•ê?ïà/Hdj?N¨e@Åõ?@Uï¶(<?"΍"!?kÑU
ö¨0?NOœ´+Û?ïÛbr¢-?eN'w)@?E8CÁ¶?5к¨N¤?oO|AÕo?cБAú'ü?ïŒý~ñL´?‡Ûõ'<Ž?E 1¢ˆ*Y?W£½‡_Ý?‹f52üR?†Òҁ^è­?ïU¢®ì6?Ue(^?_\—Û&uk?X8µÞj?"Uà¦+Iñ?€]ý8å?ïœ ³"?m›`_c'N?YBÍQyfÁ?E—ƒ"y?…ÏŸ8_¯ø?m^ú:UAGN4FGL J0420.3-3745¿~šã*86ÀFŸ}At>–À9?q/EÀ<Õ]•@º–rȟl@b:îéW?­6(ÛìOt?¯
nݝn?þr!+û1@ ³0C"ª¿Ù€ÉS›ˆ‡¿â/2ÝøÄ"¿ãêÅX.•¿âIáf6ì¿år{Gžû¿ç¸W)²€ñAGNbcu3FGL J0420.6-3742NVSS J042025-374443?ïìFÑ0ðÊ?'Þ¦.?+mÑsë1?JHâÁà d?bQâH{™?€¸M[¡ë?ïä8<-x?l§6IÔ?7^ððZ/Ó?DaFÛø_?hÛå¤vÏ?hê~.ö4ë?ïÅc»ù?hïýä$âÍ?Q&–¬ÿ ã?F¯däG?y5(q´[e?fߑ##¥?ïéãz}
Œ?F3½â9kã?<îì0S?!ÈiT(A?b™Âm}"í?D=N"*i?ïì¢õó•?aj"mÇ?)¥æ2"FÝ?"üŸ»Dœ#?aÉ®rJG?`y¬."±Ž?ïµï!z<÷?"½F@,ö?D‡\$wí?V>spIšý?;ÁØÃ??ƒm"¶ë‹í?ï¤0azKÿ?tö÷´%7Ò?X¿"º
dŸ?L܋e£ˆ?ƒÛöùUÀ?sðé2›J)?ïËÇÞ
?e.f2¢‰>?Qqñr;6X?@ØÖ£>ν?v +°9D?bÝ´×ZÀÑAGN4FGL J0421.0-0752?æjô ‰ôqÀBsUïÝìÀ:š*
ðƒ‹À<*ºè@ä²hG'@äŠ=Ü¡?Èö¤Œ'É?°o炅¬?娑¹ÑG†?ðõž,Á?ïý
Ú7¿æä¶Ê,	¿å §ªÔT¿êƒÈaƒ'½¿×8À¦MÝ¿ïü÷™Ã
AGNbcuPKS 0418-079?ï VÁF '?˜¬È
öG'?`<‡‡(ÁÖ?pµ	9Í»?™í–é2€}?—­S¡c?ï2÷ÿÞû?'Ï uQ¡ï?xüŠK¾/~?€KæhÃMž?"aÝv°cõ?ŒlyhSÐ?îdaòõf°?•«½ôÇ܆?"?gJJ|?"Ò)b"?¤ªÕVÚ?"Ó(™lÇ?ìáÌ~¦×£?'ì)¡s‰Ž?Š ¥Rd›?sÖ'Ißâ?µ®×öŒéÒ?ó ½rŽS?íl¡z¨V?±ÈÓ°ü´?s';ÚSO?'þA!47?³aÐmí΍?±dkI›6?í'R*ͼ"?®oPÉ/Ú?ð@¦U˜"?˜âò©/?®ÞÍ(²é±?¦€t!Ã|Ë?ìðìéÅ"?¡"¯°t$?•ª±\`?'(±ng?³
ì\&?Ãœ…-è ?çÙ¦SU+o?©:£\>ƒï?Ÿ=;ŒØqð?2†¾_F™?̱¿?Æi†?§˜ÐjöàAGN4FGL J0422.1-0644?î´–­^¦ÀBäâmHÀ8Ïk=e¼À;ØyªæÈ÷@mHS*õL@¬¾9Œ?¦-º<@;ô?´ÿ+Ä©èœ@	†Eÿ¾'@¨=?üoR¿ÒÔÂ$'Q©¿âýÄMc`¿çpÄÜ=ƒ¿ç.³Ý¾n¿éÚ¡oB¿ïÞfÝڑ1AGNfsrq3FGL J0422.1-0642PMN J0422-0643?ïø+h{?CÒ𱡾_?,‰©^…ý?&yH¾Ð?H1'—Æ??¾ÌM¯¸?ïèô5Ïù0?e÷Eÿ6)#?0ñǺóR?:cO÷M¾?dí'<`—?d•BëäŸ?ï­_è%¡X?{ô@º?\•¹!‹¡M?^{T©_hP?NħÅò?y'·:c.?ïú€ûƈ?*5êŸÜ·?°)pë©!?iîÕ/ÿx?BÆ
™H¼Ò?'Ì"'Xü|?ïòK¬L9?Mšê7"ú?5‰¥XI'?,&nrøT?V>9'¥?J‰UŽQ?レÒK3R?Å‰"ZH?J\=†<¼?cQtÿ‡?}g9Ì?€
·þ,jë?ï|Y
Þ?ƒ".CÕ?hNÍLâL_?jxpìô?ŠÖ
(ÆõR?'S'îiˆ?ïò«N€t7?J2¬º¨¿?0õu—©?$Í­/"¾ì?Vl¤¿'?G<Q.AGN4FGL J0422.3+1951?ïÛ=#)®XÀ4œ!ÄuæÀ9òQ~wÕ$À<2¯È@ 5;K/©@m|:
B?¹Ç¿FÒLi?‡ Éû"?ÑÝVlGQ@0fšhÌr?ïÁ¢a¿7¹¿çöÿ.=*¿â Va¶~W¿ÕApx8 ¿çÑ@>ßcӿɤCZÃÆAGNbllMS 0419.3+1943?ïë38ÖO?WWhÉLw˜?2d¤
b?%¡àóã:?bŠz•	*?U««r:¬8?ïەÅyœN?pËäo(Ë\?:Ì•»!?D*¥€Äq¢?pˆ]~0Ó?ná#ðÄÔ~?ï~Ä>€;?½NÌ?]¡+§Ú?H?^S÷È-¡?ŒÅ©ˆs-T?%dH>?ïT˵?m¾ã×]¥õ?a§­$Y/U?CHÊ°"€™?"J'•g‹?kîe¦ˆw?ïØ.'td?iº÷ú?FñO©sS?>Îô£iÿ?q
"Âf	Ô?gJfE!NÝ?ï§,{wßN?"ñ3{°å?L×G3ÖÞ?_LŽQɘ?"gl¨¤>X?ƒwÐÜ4t?îôP?'¨>ÅZ	-?l|^nü?q<€bà¥À?ìš°`~?°oî&C?î)/òÄ?ˆJüá9+Ë?ygp‹["ó?aÐ!X#ßW?ª@ÐÎJb?‡0©ë÷4AGN4FGL J0422.8+0225¿ïœ'üAY'À?.¢ ©XSÀ:?Ã<*RºÀ;óvñÎäÕ@–7t‹m1@
'¼«ì?ÎÍÉaˆ[.?äN.Km@ Êƒ@¬Lfn¿ÌmÆWߦ¿á(qy‹¿ì!yÍKwοïø˜'˜K;¿ìl5恿ï¦Ñ€ìAGNfsrq1FGL J0422.1+0211PKS 0420+022?îeE))ð?­ù&¹x?œæovŠ"Ò?ž¶¥Ïû? fsñL/š?¢.òTo¸?ìõñ¼,—?±ŸØÌ*'«?¦FÌ+âé?¦u5ô%?ªˆ¨Õ}ž²?£c&Šª?é¤jp¿¹G?­V]‹Ÿ¦'?·Õ$DŽír?¥PÉè‰X?»ˆ4—a[?¤Å%n¼…´?ê®W™ølÁ?›–<<Ó7N?ªA}-:;^?‰¥IRû?½l"–/àK?•éˆj(Z?ëyÉw­¶‡?¹º.,Á²›?±ÃŠc-½L?°OÖ5?²n)Þ³þ?®¤
fË.?æÓE™+#‰?Æf{n$9µ?Â÷9"Ó`?Áž!Ø[»?Á»°Þ|?¸q?ÿ¼'«?æ쏤*ö?²êG¹=~?ÁË]:\Œ?­v‹©j=?"€‡È?ªþÇ ?áï"Å*}=?°úVϘϲ?Áðd›Nê8?¤ø¸Þÿ
?Ó(¦&ð¯«?¬Tþ;Þ>AGN4FGL J0423.1+2106?æ¶L:@B»À3§ÑEØQeÀ9É2ÄxjuÀ;鞍õ ©@ŽÅ9°zÝ@#¿!é_?»Jm·hŒ†?³ôÓ|vÕ?ùÝÑ6¾Øî?úO–@HÅ¿Ø¥bïڿهã¤)Àn¿çù‹!0Ò0¿ß8÷b¢Œ‡¿å·a¿ðAGNbcuTXS 0420+210?ïd/c‰¬?ƒó!‡#Ÿ;?_H&+ƒ&"?Q§±´Ïr?'…'.N¡?ƒ#¨ë³x?ï);æØM?"=Qì&á?µaY¥?‡øßKëÀø?'ýìzH7Ö?ˆ «q½š?íÞI®Â4?š?݄À^?t˜q`?‰abˆšÊš?ª8ìÿ	o?•9 wwc?ë«-oò#?'?Ý	Üò?¡aÌzvщ?}'zÀŒ_?¹öPSÕj*?Ž‡,u"·?î»m†b§Œ?–ì–õ-Ë?wÙû–>Ë?o—3&ҍ?¡Mè6ÒÓa?•@¿;Sc?í,8¤r?°ðs¤Y¿?žp®îßT?§e7Î^®?®(˜€Ú?¦ê)ÒQë?ëÆ
"NgR?¥ B¶K¥?›5‰fÕþÎ?Sæ'¢?»1iR:?£+<÷Z©•?æ&#lZ‹?¥g"ìiF×?µΛ ZÓ?–5ì˜f‹?Ìߪ"×?¢‰üÙ´AGN4FGL J0423.3-0120?ëð\aC¬À@>}QÀ8
g†!ÑÀ;Á%ϝb@•,]@ätÙÆ°S?ÆÅÝÖp¡?¶˜W¾òˆb@ôaùð†@uÏ¢<x¿Ó;ž̬¿àO8añ6¹¿å-F¿×ñÄ¿åâ;Ÿh¿çèµ@i&µ¿ìsüPHAGNFSRQ3FGL J0423.2-0119PKS 0420-01?ïæ1f‡@?a¿€ã+ô?97—7"æä?0ŽÎ©{?f§}¹e{(?`…é	ؔ¬?ïä}F™?gê;" ÷_?;‡ój7"?NÞ£;2™?gÿ"˜H;N?e¦Æqt§"?ïÊã€?r1)ë~?Z¸‰_Z%?i
ø?í?sàU8>Qt?j€>ƒ8N9?ïùfw	U?1ïÖS¦-S?ö¦Š§?
	ápð"?G
ª©Jû¹?0]Ό§4î?ïÒÆXG?m¼È¹êâT?5"†yší'?+g×F¶Iñ?u™äŽ#µ?lí"NÙU?ï²¢ÓeS}?'Y#^á+8?PøÔ¸Z?h‡}`ž"c?8I\:Iš?€–…™ƒ³w?ïÅxD+ËW?v܀i´ß?Zá¨íš±?inð\Ωó?v‹,¡Ç?q§ì"r«G?ïñey+1?LO˜qO`Ç?-ƒáك`ü?!}Ó}m1?Y…Zcøô°?JW\ió,AGN4FGL J0423.9+4150¿ëÊ÷nN{À‰äÁ¶UÀ8X-'JTÀ;`e':ØC@¯L$›À»?üƒ3á®Ü!?¥–˜Þ2и?»övÿ»·|@Áv¹Ã@¿úQo¤¿Ì«¥'[¿ÚÓ³¼¨†¿Ú²!$袿ÔïÂ',j¿â"n!EÊå¿ãÛG¹ÒõAGNbll3FGL J0423.8+41504C +41.11?ã€t…±¡?½š¯Ì¿ik?¦Aá¿Ö¢Â?žÑêЀÒ?Ö6Ú½PX?»ÁœuŸœñ?ÕÅn5à-?Ì/
¾ŽµT?Ädª[™ë?ÁqÉ_É­ø?à!zyï?ÈĐl?ãìÔ)7†Õ?²×úËø6i?³7é^$ŽÛ?£)K‹–7?ÓX]V>È_?²9Ü$¤{?án
õ|?ªyä2?º÷Ñ:ù?•WX芩£?×YˆåõÆI?«‡Ðˆ2õ?ØÂ8ÿÐÛ$?¼JÿµÇÅ?¨7	#À?‡ýŽ+iu?âríæÖl?¼ÿ'ÐZS'?LJü>»Æ?ÆX<äÚ,(?ËÈ""uå?È¢'dì¾°?ã+ùˈ?ËÐ"qîÑ?à(³†äz?·€5'°‡¢?¯²}Tå@©?˜ÚçH¢Q?Û¸IGœ¡·?¸'HÌXÌ?ÔSäúÒ)ê?®]'G:?ÂHF¸?¥'ï¡Ý¿?áNp…=?³'¢½û:ÙMIXED4FGL J0424.7+0036?׌)ù"À?ÆñVIÀ8«ü†Î»ºÀ;Ý[o'_@Âqû@JTFŸ?§£aÍ/?¬îÄ$÷J@瀕Ó;@S¬½¿œ¿×Õi>!²¿ÚäÑ@±¡¿ä…péP'¿áäø¨ê¿æFV[Vgì¿æÖlÞ¥'KAGNbll3FGL J0424.7+0035PKS 0422+00?ïí-/c?Vp$òÿï•?-7qů¬?#k[R?`ÿYN<Yf?UcGšÂ½?ïÊE •ƒ­?zd+Q&3'?Jì(|Æj¾?X×MÁkP?wª¤À©}?vÕ`-ŠýH?ï³iŽ[o_?wq±iã';?_U7åS'2?lœíMÙ!N?~uêãB?û?s=;¦õyÌ?ï¬s²ÃûÝ?aÙe>ϚÇ?dsïáxõ?H:,æhgú?Œ.ÿtMZ?\BðýC<?ïÑÚ¤ëv?låìã«|?AåX€ñÓ?7<™‡›¦?tÖœŒ¯N?k 7EÐ
†?ïeœ[cÔ?"¹¨ô#«?_5M—Õ?p7ÍÀHu1?'Y*Zõن?'n·"lÜ?ïˆ%ÓE¯.?÷‹'æ?aÍp}—ã"?e¤B/6d?‰ƒ/
^Ǚ?€h,­¾¯Ë?ïE#²#S?_ÝÑ¥ü?xÁò²qM?d-ºI¦µá?'Zl",;?xž=nl8AGN4FGL J0424.9-5331¿À¦\m
¼¿ÀEÓEŒÒÀ9­ß…65FÀ<A»±–^@Ź'Fî@"
f‹OT?±®xßöÜQ?½U&^Iȇ@
ÚXÁb5@×Õ?7"¿—I›ªjø¿ß,>ø8`¿ã+åï¿ã0AFmD¿ê¤E>Îqè¿ïþú|2€†AGNbll3FGL J0425.0-5331PMN J0425-5331?ïç?p'ý?V÷/Û/?Dq{‰p°?9€¯OÃ6
?c¤Œ›2™?Raâ±°"²?ïÞ "Š'?pÖ[]Ë—?<‹ä}Ì4?I›W¢n«<?mÎ
KÎ?mRNPJé.?ï Ìºòôn?vå
@€»?r*sºð}í?{­L÷Ðì¢?}o.äR{&?sgS©#ë?ïÞðE\?H£µê
Æ?Fy6‰*¯D?+€lÊþ?kqmQÑQÁ?DëÚã6C?ïÐüR"U?eYE«'½œ?SQ3¤Ÿ='?Hô‡d¥¡©?r­dX@r/?bjûrcâ?ïœÕrÛK?ˆ[ìpô7?SCöJ[+?fgOŒªÂ?†b1e]Ö?…`¬â"~Ã?ïaÒ¨ƒí5?‡è7C?{ry²Ý4?€ø,ÔvÉ?‰ÒôÀ??€Ãw'§m?ï³<ÓV:?eꨬéKî?Z*bÔƒ?FÄKIõâ?èI".cK?becûˆ½AGN4FGL J0425.3+6319?ïÐrÊf°@#‰ù&ÇêæÀ9ì
±™kÀ< ÌàîÂÁ@!¹ññIƒØ?ý_ñ7n+?º ³iNx3?"êxg«ò?Ø©ßAÄpˆ@ò`gžÊ±¿Ùž´@cóE¿å®Å"T¹¿ç¼=s(¿Ñ÷†^ÔKÇ¿Ó\ž¼n¿ÚæØ;ÀËbAGNbcu3FGL J0425.2+6319NVSS J042524+632005?íÆÕͅ!?µK"S
Öô?Z‡‡hª'v?P=ã&"?±_3wÖÅ,?µBV òM?êãú>'¶†?'òï\€?qA´\;á?yŠÆø4u!?Ãç<øâ]
?ÂJM<Z	?í@cyeáJ?¡/—¸¼÷!?w'˯û_¤?t¨6†¢
Ÿ?´ƒ·{1³?¡=wÓO?·ZÓ>?†éì-ÀK˜?s'¶ßµÝ?Yµ<?§Üè?¥QÝÂcHl?†ÑÓäòr?ë:™U?ç:?·àÁDŽ:A?rrٟlº?fñŸïcð?'ݧ‡æ?·'†ÎèeB?äd¯Ïw2?ÍÅ砍©¡?€ÉRb,(Ö?´½¹î‹?Ö±z
.´?Í@I?ÓÄR?éÖX¦#.?«ð­ÄÍ8¨?Æ/̎Êò?v4逹Z?NJ:k‹¿;?«ŒÁè'?ë±¹áì!Y?¢õ¢í ïß?Ž^kê5¯?€Åa+e ?¾¦ct¢ý?£`›"×õÞAGN4FGL J0426.7+6826¿èˆ€•ìÄ@*º=ú	FÀ9¹ÏµqfÀ<6¸©õ@!lµàÍ
@˜vƒêÛ¬?³¶ûª0?ª´Áp'ý?÷³{?D@yáSígø?ï÷ó¡Íś¿à³ŸÕý¿åŸ+ÿ¸1Š¿à! Ï¨¿ãPW›ÈH¿æ]4Ž}åAGNbcu3FGL J0426.3+68274C +68.05?ï®øšŸÂÂ?t7¢ÌzÅ?T"ÚÃ*<?F¾Z\4kš?¯^e¾?rt»ãvT—?ïnÊ+:sø?—¯Ì&µ‰?a‰aVžÕ"?i¨úñ\~?ëÎTÒ¹?–6ÐyÇÆ?ï|±G"?ü*Nj¾?b©­á3?`óÄg-?Œ)XœÞð?~‰i‡?ïÊUÏ?söp9~?óûÿ"ö?[Îý²}€0?•H¾j?q¢‡D#¿?ïKº¾'\;?ŽìPíû"?eú]Ê%?ZזÔì?"Égª˜¡J?ŒUž»t?î} Ö5–?¨'®ìðŒ?yT†¼ˆŒ?†mÍÄ
à?¤ûaŠ !?¦¹X­"n?îîÜÇõ*B?'' ŠuJ–?qÞ5·;Oë?n§;ÝŽ"?¬Ù'XÒ?
·è.ë	?íAþiÊ@x?'~z£B?œgnbÙõò?}E$4°;h?­¬b5^™"?ŒP;†Ý·þAGN4FGL J0427.3-3900¿îÖ¡a[‡ÀE÷—$tSÀ8ä01öóÀ;´bTˆîQ@å†Tmj'@¾–ÃüC³?¨Î½š
L?y~þÈ#n?ʽì(2@xS/'
¿ÝՂ}ô!¥¿åÝÓð­|¥¿êœ¾™XV¿ç8®6Ý¿ïüC²\´?ï|.NÇä0AGNbcu3FGL J0427.3-3900PMN J0427-3900?ïùßrï?BüïòØ¿ü?2¶`@8²?1Õ!«»RÙ?>þ½âQl?9¯Â[Ã
%?ïÒí^u'?µ'Ð3t?E"Mº&Â?Wq-+<²Î?sÖµ¥/!E?}ÉçJí†?îјzyˆ?•ŽMÚ>ï?€ê¤Ó!cG?"ïÃ¥(u?jZ€˜Ûr?">9ëkðÕ?ïàÊžUì?TZ€¥$?F,Çê&U?3âj²+ŸN?iª®'sU?Qæ25q¥Ù?ïðr&Ü
?^`•"r©2?Iñ¥+k':?N?Ë®&K?R"+Ž¥%
?Táû(ý?ï|Ž©P›Ï?"~V–;uŠ?VȺ¥?j‰r‹1ÿ±?ŽÔáˆ	"?'ƒu­æ‰‹?îSƒ€†*Ú?žÑ
ä|
?"VÖÔÍ?†lÃ,"
j?¦b²DéǍ?›²±øÈï—?ï˜Ùéüï'?zˆZ7rÔ?g"›^ÝßX?`¤ê÷'?ƒäž³û?vÎF=áÀÚAGN4FGL J0428.6-3756¿×¦\š#œÀEέÙ©TÀ6EXôÛöÀ:©fã@È{zIÈ ?ÿë|Öt+?†Nӑ{׬?´ég,ù³@*Lˆ3?È@ QúÖ `2¿³¢ðŸ(¾¿Ú#¡ZX;*¿â'°âÄ¿áýˆV{7¿åé`F'µ¿è Fý"5AGNbll3FGL J0428.6-3756PKS 0426-380?ïÁŽÚ‹Û?s˜Ó¾‰A?M%-[¯?LÀM¿Û'?{†Òøvýð?rDjüïÉ?ï	.nõ£}?°‰î¹ƒ/O?uÐc9öâ?"fÊ|t÷?™fU	Éb?­h-ÊjQ??íþ /±"®?¤6"•šö*?'y¸¶fð)?"''"5ºI?¦á ¨ØV?¢=OGºŒ?ïUi>!²?ˆsø±hS?g*7"Ñ3'?d3ý¿#8?'m'Rù!??"ºPÀ¯)›?ïY·Ãj[?…Ï܆/-?açM'šô•?_Boð¤a?'Œà.·?ƒÈfFí?î:¤? 7"?²lûÌÔ&?'ß¡lqü?'öUåÃF?§ô£ÿ™Á?±DzôIÚ?î,V¿?¢=ÃÇÆ?‡u«¯š¶?Ž€‰I·¦l?§aDœõÁ#? –(‡Í_?î^™¬ ? V㣔Im?wZ³å~);?t,y™e??§+_+æa?ž Õ&ä|AGN4FGL J0428.7-5003?ï<)scFnÀE‡0HAÀ;O¥^ɹóÀ<ˍg\/¬@í
¡~?v@"!4x®?Î×^v-í?¼/'(áö?îŠÒŒ)nŽ?ô†ùç71E?ïþ±ëÕ¿Ò''Û'‡¿èˆ¥@ï«¿ß'£G˜E¿ïÿŽñ ¿îxê݃ÿ)AGNbcuPMN J0428-5005?ïiïú=72?ž¾¶HKÕ3?eÇ>bìR?–m+ƒdē?	I­"C?•sO`˜ú–?ï*'2–Lª?è{e7M…?z9ÙŠ'&?|Ä2…Ÿx?",£QGS"?ˆÿpæº7?î>Xw²¶?Ÿä,$?ˆsó^?‡JçÐv?©ÏTw·­½?ž&lÈØ?·?|§–Y´ù?'ÄÔOÜ?rö3üCv?—#iš+Ž?s}Ð"J?ïvš¹Ýºc?˜?Ðsªö?QB'o}.´?XçÆ=ž=?€"	î³?˜+î?(Ù?í»àûÐ<æ?©DRè ¶ñ?1d]°?—ÎA´-Ù'?¬u—*ÛI2?£?qYÉ?í˜oq–´ý? '0èÈY_?Œ€Ös!‡P?Š-ž­ ?¯XÓF\²h?Þv­`?ìĄÈbk?˜kÈ©f;)?¥‹8‡Ü~?§(Õ4šÿ?®,zó–Y+?''V+7AGN4FGL J0429.3-3238?áh$¬ÀEzšu%FÀ;G\WìÀ<иãá¼H@P¦?p?ý™¨bŠ8Ô?ÏN×(›T°?Éó˜Ôw¼?ö1ƒ/ÊÉ@_u†iç¿ïü.ÿò¾ú?ïÿërªAˆ¿Ú#|"jÞ¿åÀ¾/@¿ÒéûF\Û£¿é*°bˆá;AGNbllNVSS J042900-323638?ïÉ?e+äñ?oõFåhä?H°äã¾±¤?;ÄÓ=5é™?xJ0è
®ð?n¨ƒ^E7ô?ムúؒ˜?|XáºçêW?HÎ^3;ŠÌ?P']@P?}6Ó??zVÇ}є?ï~öLšZ?=`VيÞ?s¦@±J	>?w¨@ãŒb=?—†'fõ?Š	1c©#?ïNÏpëû?hº—'½Ëà?^!µú#ÐE?EªÕZ߂5?‹è``ÿ$?g2.ÀМ½?ï–Ån´"›?z«<,ù¬®?^¿膧P?Te s»Ø?†v´PúÐ]?x¡Jvqz"?ï1åÙkÊ1?"Žd¹x
?]7,nH_?f^ ËYö?—ò'^_ýY?"xªãMT¸?î¬È¢"	Õ?'*˾V~?zÙê¥Lk™?|'mXÍz?¡Ø8†qX9?Ž'@zˆK,?îЉkŠMÝ?ƒÝ…`	?iF-{V?)?\ IKÏg?¡cmTº?ƒ\>Pdõ¸AGN4FGL J0429.3-4326¿ï¾û¾°]ÀEÅõ@‰]À;å(
eCÀ<¶ýwÞ@bå®pg@ýø8‹?Åê•_£(º?¨ "ûé¬?àÿG¾…ŒF@:~6Ë¿Ú&Gݏ<É?¡9À–¾»¿å§ûâd
Ç¿ìSå1[¿âWÝó»¤?º‹¤ùÜAGNfsrqPKS 0427-435?ïÓØ¿Ën?kÙK[)9?5Â
v‡Ã­?3Tà>7à¬?t·Óig®U?i«ýÒrç?ﶟ,'¿—?zþñ%´Qü?PùyÁsŽ?V²ì,k?€9ªðÌ4?w
Åóî
Š?ï.άmS7?†°yu?o¿ÍI¾B?s•äb¨‡A?–.0ԄS?"¸ÝáÚìn?ïλ¤R҂?T=4E"R
?E­…;X?.#6TV"?uìŒ:Íd¯?S¥»_ÂÖO?33Ö?ƒ´ôܽÞ?Gˆ¾ÄQ'¦?=3!"¤ý?‹!¬üaŠÁ?'¢?¿5p?ï>Pýã4?˜|*ìêXâ?`¾¬Å8¸g?nDn$»î#?–$àJˆ-n?–B[ 5uE?î€
–ÖN?"7ëØyk?{J$Z$?|§Ç<9¡?¤žMV¡¬ ?'Âã<å^?ï]ô֒Y›?x
ÌÒv?^u'"§›?P, ڕ=?'Z½iNð?wÚÀš€D—AGN4FGL J0429.8+2843?êi5úäÀ*óÝüŸù/À9RîؐOnÀ;ÃD°E®@½?Çk9	@` ßs˜~?·‰Hh¤"?¾Ìևá‹K@¢õ:ªú@5PQQ+l?å$Ã9¦¿g¤Ò»VáA¿áhçv¯Š¿ÛuÓáéêj¿äï ×{|x¿è	çàN‰ÑAGNbcu3FGL J0429.8+2843MG2 J042948+2843?îßÛ¡:Ý?ÁÈÖ!yQ?˜8ٗ3Ùc?Áôõޜ‹š?‡—dŽ‰•÷?{Ùf0´w?îʗwo<?¡ÿ¾(ԑf?}ñðp?"5bÓØÜZ?—+Ò	S?˜Ç«Ú÷£^?în´"Œ'?•‹"A¾r^?Ö4ƒV‡?—oáþ@?¤Ÿ)­KÈÃ?'.îû¬Ñ]?ê"õ™°ÑÖ?'bz<"ØU?¬ßþt8å?€®¾ÈëÕE?À<)üÓ¥¯?sT½Då$?î^
÷dz?·Ôþ§=Û©?šËˆMB³A?·ð¹	M;?™s7ˆT?‹ZÕ¡x.g?ìŠÃ"²?¸H™Á°Û?¨zéø?°p"­`=?®Ùµí¦ûÇ?«"v_šÕ?싨»S0\?¥*µ°,^?'û·\RZN?Šl7§/[?¶ãÌO›Á	?£–Õb%A·?ã§Ræhš?¡® rîãb?¿1cVþŒ?™&%ËÄù•?Ðåqš!)? ‰C AGN4FGL J0429.9-3101?ÚpÃÜÀEIË>WS¤À:&˜Û-¸ À<r$ëqÔ@!uƁ?ýJ½"så«?½¾¦Š˜Ë?»×xÍFD]?þv‰Ê½f@Ô:®0?ËÍ2xMC«¿Þ¦^c™¿Þí,¾¤ëÝ¿ÓPNâf<¿äò?£%¿ç´v)RáAGNbcu3FGL J0430.1-3103MRSS 421-156568?ïå$Êå—?SÿÉ´Ìs^?5,EÀjõ?$:gÎ|›?hGROF¬?R›Ñ[§x?ïÌ$¦uS?t$Ï H?F"mH¿?LïS¿ŠkÉ?w)®N?qÓàâ]ú?ï›-.¯?nÎwÜ­Wù?\‰µ
N®?^+´Ìî`;?…£}$"?i9PœL?ïsî=$°?b7ªQOæa?eºåóP ?BÈ%+è'?•·1¼ý?`Ö7¸ˆ²?ïÍ.Ú+?aÁý"ü!?H#ì>uh?6àh\}ì?vdv™†Æ¦?`FeæËé?ï[íÍ´z?™Ý¤Dõ&?Zô'JÖéŠ?jCN]¶	?'Òþ"ò?•¿¦«
?ïIë?ïÃ?€´¡Æ°q?g K:k)Ò?aJ2ä8æ?"ÞŽµÔb?{æÒàÂÒ?î¶tñ™ŠÖ?~ÐúE¹B?wÀ[á»cô?^›»Q4.?¡ ¥gÞ)¤?{JbÒ·¦AGN4FGL J0430.2-0356¿Üˆ¨^óWÀ@}7\ŸÀ:ÖöV3|À<i²?'ÌÎ@'¥e՜Õ@øá…Áu?ÐRVy‰XÚ?º¹»£К?ä¤Váä-@	ÓÆë|5¿ÐbH_bŽ¿æ(ºžÌßA¿è,PÓ¿î,ma,j¿Ð|T¤Çõø¿ïm í¶QAGNbcuPMN J0431-0406?ïû<±âÕ?:?O>јC?
œÛA?"vš›{?AlÏ7^©å?8£~ô@?ï¾(röþ¶?ƒ¡­Ι
?NHî6oB?\5ÓMNÐ8?}"¨¼ñ9H?TiÝÀð3?ïvtUÎz?'&ðÍ	?]$š¢ç?ißçê´?Ž·>^ú%9?€RT:.Äø?ïçW$V?HcÕƹÓ? á. ¬JZ?²à— Ì?gšÈ©3¸è?G¨¨‡s~^?ïõkÂÏP"?QçaÁm {?ØFÉ¢?HiÌ5½?Sßz ý—?QW`÷»?ïJ¡Á 
?™³†>mÛ?ZT²Î°ò?m§ÿ¹5L²?•¢žBN?–k-[¾þ¿?îë$,)?I¯ÑˆV"?fhQ:–½?p›Ñ8¦i?ŸÎe¬–Ç8?ÛL̟Eú?ﲍ1"j?jb;Èù?4vP ‹?*ŒC®8¥?'¹çã¦?jÛ/ç¨^AGN4FGL J0430.3-2507¿ë\'YèÀDFÜ]cˆÀ:0%°"±"À<z"UŒúO@wàÎ'.@0ñ¤óið?¹^€hñ;?œf8n0Š6?ã5Õ¿º•"@¬7ñ³â?ïò+
0À¿ãî!	¿â¹·a*½C¿á;w¥S¿ÝXODù"¿ðAGNbll3FGL J0430.2-2508PMN J0430-2507?ïÊîÛaÝb?g™mÝ"ºP?P/ÀåF¡?M!¡hÍ?v|Ëëh"?e;n¢ÁQÂ?ï¦JpLÕW?Œ†•l`?Tþß'?X5á]¥?ƒëÄÝz?Š½P?ùä4?ïDr¯KÝ?"²'/ò??uA¯`û¯?|Ö±O]S?'!S8–‡\?|õ诖X	?ï]ó'ÃÈ}?m'C§ÿ×?k•s`e?Ox‡y
®?Îì\– A?j¢b°ÄA…?ï†À¡è•?'ø«–Ôê¿?kpŽHô?ƒg¿\â?‡"
r<?{æ}`E•?ï"™æ¬®?•7/¯)ª?bԏí¨ú]?iñ@ɬ"?š2ÚÌ(‡ë?"ÑñRQ×D?î ìÜ♓?ïU9¢ ð?'F˜¢Çj?€uÇ«§¤?¡_Œ	fšº?ŠÍ‡úä ÷?îOò§Z€?ˆë™*XÐ?'›ª_ù["?mB%\DŸ?¦Yêõ/V*?†gÄéøƒAGN4FGL J0430.3+1654¿èÙɂóîWÀ5
ȁäq.À9—ˆŠ}œäÀ;ÉLíï\D@dƒÖcÏ]@Ŝ[cÔ?¶#Ú$ÏU?šƒX ¼3ß?ã¤Ô•îê.@ÆîÍӇý?ïý³õerK¿ƒ]$ԚĿæéu¿Ê°¾¿ãڛ!Y¿ãxê݃ÿ)¿ç}d¿È,AGNbcu3FGL J0430.5+1655MG1 J043022+1655?ïÛõja?gëú›"Y?;þ‹êH¶?29©œòß?p±œ{¾jÉ?eÞ¯²õˆ?ïÓ.qÊH?tdӚŒ?B•ªßMäK?HÔ¿ŒèUÛ?tIŒÇÔ?r®–Ûá¼?ï8€£d¯¾?‹²=#üþ?q7iÿp?vʞV
D	?"‡‹¾ÔU?‡ÞªÚY‰P?îñ:%yk?tópŒmŠ?qóÜIx4?PÚyæÒX¼?[ök™»"?s?.žëg?ï«Ðúó•}?|ãFÂœ?T¡æ~S‰ì?O/Gà?'w"n€»x?{«<¯‹?ï†!mMû?ŠV'êÈþ?VÊó¤+?bڃ›ßD?‹žazOn¬?ˆZxů9N?î~¦Œ´É?™
ƒ¢i?6®K°9?€"ùõs´?¤.Á\Ì̱?–nîP-?í2%±aÙ±?½ j*V›?ŠD-ˆL¶?pÞp'J.?³)ðß?ŽhÄÈC¦AGN4FGL J0431.8+7403¿²íDkEǀ@1^‹\¿ôwÀ9ÿ¦å²vàÀ<oLjÀ-'@ýBÝ ?þë`ºU?´åV 9Šª?¥8iRÿ×;?ð£~õ©e@fuÜ{ ?ïÛS]u&¿×^Ÿ"¦¿ãû–yS¨õ¿ØaéÿãzŽ¿Ö•ǶãV¿èÜ)áû³AGNbll3FGL J0431.6+7403GB6 J0431+7403?ïî\'ÉÑ?Sað)°?3TkMЯÍ?$®¯ãН&?^qàÜXo?Q®l¯i±=?ïß«B¨5?qÉv´=>?BQtÐ!dN?N¢²Âi'_?kÀ_îµzU?n!A8š~?ï´Ó"²Ç4?r‰Ùñ@$(?RÞQ$üâ?Ro»Qâº7?€‰FiãH?q¨Î`5ÍÕ?ïÄéWX<¾?X"¬/€n£?U†kæ?Q?5n›kÄ©?x)¹9UŒÓ?W4%kˆZö?ïåJiÿ?]g­"·^×?@C"-©?0.B®JÎò?fø%	ᕆ?[Ålõæ?ï¢
—õF?†…Ÿon?Töuï·ö?cf/±ìX?"ÝË{'¹d?ƒÑôÀ6'?ït;.\èA?"DftR‰?X£ñx´
?O"ïž@8?í?Ý0_S?ƒ³[œfÞ?ïXí_œü-?uW*í•w?n§ýÿ¯?WT	Š?'
TG%<?sâ`ÙóʒAGN4FGL J0432.0+1732¿í5kÈ·$«À4U.ÓÀ:ÆYåN£ÒÀ<pz¼^À@îQ†…j¹@Á]¥Í"ƒ?Ô'øR¸?Ûß©~+V@µ;ÑgfA@"pµßö? S~œÅ¿å(Уñâ0¿ÜÚsÿV6î¿çLê"]ðv¿ï»batE¿ë¥­Aí
AGNbcuTXS 0429+174?îaáÎÞí-?¢í‹7šå¹?ŽKÞdtª¿?ŽÉçëQ?¢Në{‡·y?š?Ía%?îÜ<×Äç?y"×Æx?‡_™U—…D?ŒÌñcCÂ?˜È²¿c
o?•¬ ¹:d?í;…'œAŒ?¡€"<î¦o?¢=Š ¯í?–=gTýý?ª
^®ìO?–RÇ,ŒÁh?ê¹ü\ÿ­?—uù†ˆ'©?'ÓïtÐ3?ri\CY'_?ÅNš"j?–œKeh˜?ìÜ@!?®¥•Þö†_?£ŸÕúœ3•?Ú¦Ø†X?µ93`ÓB?¦Næ2ót?ì«Dü">³?¶eU^ˆé?£nد?¬Õï;Z˳?±!Ê2?¬®KïAÂ?꤃‡ß\ò?«»tæªñ?°¬‹àY­­?¡Oañok?º/Wà«jÁ?£€
5Ût©?â½Äï]ÆZ?ª?꿐Ÿ?œnu#yŸ?‰"e·›¶u?ؽŽÏCÓ?©ÿÐE­RAAGN4FGL J0433.0+0522¿ÑhžFsúÀ;j¡è´lÀ8ôxmÏç4À;œ=þhP@4@§ºï€@st¼j~ú?²‰`
0ë?Ðý ¿¨¡õ@×õûn@…¤Q¦ù¿×›X¶z{¿ãìÓu]¿éÏ^âäfG¿ìª$Ìh"ÿ¿ð?ëí×^v-AGNRDG3C 120?ïÀPÃo‰ƒ?ÒEÅw'
?m—·˜èV²?pó¿œ	ûÊ?q""ñ?x8êà?ï֕¾Ì6­?w—·}kvØ?Iijyhx?YP—QÕ²'?q| [é¬?sÊM÷?ì¼OÁU¢?¦ÃŸ"UÑ?ª&ÂaŽæ7? ¶ºà½ÏÂ?ªA‹¨¤«?{•àmÉ?ïÒ¨NÆÀ!?]¬Ìâȕ?K—i­n u?7à^–»O?s8ëX¦þ¾?ZG{VÇé·?ï…àÏ/Ÿø?‹>΍eZ'?yÜ&w/+Ó?€®1
	š?™¹g†?ƒ"àXV™?ïqPìñI?œ"Iv!·Ž?fX
JOá=?…ÁÆo¡´¬?Ž"(dqEr?–yÇÑ}?ëŠX¤íñÇ?­\u¹ÏöÌ?±iÈ	ˆY?¤#íÆǙ?²"ÑbÐp?¢éÎa½ö?ïXzÁxl	?'˜qŸ)Nw?jÏô~%w™?]xt݁ã¶?'–©:¦Ž?€¿g)öñ©AGN4FGL J0433.1+3227¿È"°êv´pÀ$åi+<ĬÀ:7®_ú;›À<(<üàÏ@!A¯à+#?ýhò	1?ÂP?§¿!?¥Ùr€-À`?ãn;¢BŠ"@ˆ™úg±?ïìŸ/ۏ޿ê.8!¯}1¿á¥îaG¿؟Úép¿Ö
µ%;Mß¿ç› Yý!AGNbll3FGL J0433.1+3228NVSS J043307+322840?í2Aèúø&?¬ø1û0Վ?Z¼íéø`µ?M~j$ž?¶ýY'?¬Ã4ÙmÈ?ëÏ¡Éé?¹ê±¨óÃu?dp¯)ø›¸?n_ý¦ôÁ?Ào¶¥üm?¹ÿñ'T?îXþ‡Á<?–W+šiv‡?kÃPn¤Æ?dĉ6;ý?¨¿ÛQéºk?•´»¼ŒÁM?îJq£0q?ƒ–°í†s?k;qŽX?Kð‡	D²m?©®e1÷¸£?ƒ—çÿ·g?雪"Nè,?¿Q‰Æ¤?lr‰Æy?`áöÔÙó¾?É!äEm?¾Ý<0²ÐL?çXª!tß?Æ'¸"Gõ?i•˜xÊP£?tºxÑíþ?Ñ€°Oϲ?Æ	ðø-×1?êõšÆaÆ?¬+Åç¼x}?|Óí'@ãÓ?rÐ%:ÚÃò?ÃBõyz{'?«Ä힫1?ëVëI9°?žJÌMñŒ?¸ÄÑ,:?n­âJKZ?³Z\î?žÑ^Ðò€£AGN4FGL J0433.5-1039?è÷`\C«ÀA²÷üü?À;vºq€vÀ<˜Fíû¾@éEÔJ›@'µÿ_Ç?ÈÒ»y=X¦?®ßM>2{ä?àˆµENJn?ü\±+†–ˆ?ë.-9ôîT?ç­½"4Þ.¿ã&ä¦f&¿ãñV^ÜY]¿ïòbRÛo'?ïGÿ¨Â+‰AGNbcu1RXS J043333.5-104220?ï·Þ݀q?r	#z»€r?Pe)ãóÁÄ?F5ý¶Ù%?÷¯å_?pÏ"]Ý?ïz¯®%d5?†|R'kÛ?ij0՝Ç?sUÐZ¢?‹
ùñPÃE?€€ËÙ¾?ïMÎñ'?ŒÒïʪh?xw/W͙–?xg1úµ?–¸zd²ø‰?ˆB\Z™µ?ï@±Õ
ð?vc¸Ô:†?}_µ2Û?dl­¦4"K?'Ø$ܽ¸?pûßzʄ?ïeÀÔæ»?†É{3§ø,?d7¥÷^k?^ë[8Äò?Á­Úy?…9:NÔ{?± ®?¡ÓUVb|?|!A…'½î?†H9$žS?¤\¿T±a?œj'YÓ?îƒ>†ÖüÚ?"Í1îÜäi?'¶PrGþ?"
D&lœ?£ƒcŒ_?'
"'¿?íÿ¢³¡?'ÞîVm£?Ä"Ùâí?€÷á(qŠ?§£œUJZ"?… !úÏàAGN4FGL J0433.6-6030?èÜ
¬E1§ÀD5\ÙëÀ9Cº­˜#À<!.b@ݝ^ä'@¨— B•§?¨îL¤Ht8?À³l©v†@:x¯>F@¨Úã:øO¿Ëç*Üw¯¿Üp5½Q.Ç¿æM±>&p¿çÒÌ ×üV¿ê"—8w¿ïýÚV"K"AGNfsrq3FGL J0433.7-6028PKS 0432-606?ïÜcÊ>?eŒð*­M5?T²¾±¾—í?P"-±.?iC—Ø¥î?aŽñ‡-¼•?ïÜÐ$	
Š?s½h§C†?@`)àYœ8?LPk•Ùø{?oÑB©N?p›øºØ€Ð?ӃZ?'5ú¹sA?ilùæPûr?p˜ØŸƒ{?ƒ'œÃ?׈3¹B?ïëžÕKT?B4þäŒIz?D«Ž)Óß«?,Éh¶Îï?^lŽœ,a?=aˆÊê³?ï«/RAÛ?u©¨5`Ûr?gÛ@'?cˆ?`Š¥Í'é+?~z¶Á#÷ƒ?p^k'ïŠ(?üaB™?‹´m%4|e?S:e¸0Հ?hæïŸù?ˆ®ôËG<?‰z%w¯?ï]×Ø?‰"BM—z?vϛ ¾Ï§?~i³È¥èá?V+t'¼?ƒ"Þbª¦Ô?ïËCOµõÆ?a­gXá?[~͔3°\?H-y‰iö*?s~¤Ö¥œê?]àà°"ÙAGN4FGL J0433.6+2905?äzÓY?²À)3¤r:¯ÿÀ8\iñŽMÀ;9îיå@1ºv^;?ÿ²lHþv"?¨	Ê?eò?¶ÜÝæûw/@e^è¬@»G»ÖZj?ƞÅ''êN¿ÛnÂ@öö¿àobùÊ[Ù¿ßÄ-ÁÚ+¿ä!¸âÓõ¿ãH݉³r‰AGNbll3FGL J0433.6+2905MG2 J043337+2905?ïïOt$?Q'¢§m?Bö"6È}!??5ýτži?W†¶zÜ?H°m›*m?ïê'e?n?žÀèÅ?6fMÛÊb?M2µVl?b¡2h(h?kÓɉÿÂ?ï"ûý¼Ù»?ˆ¼O.Äí
?m*"З,6?z…à|qˆ‹?‡v_jº,8?"nð@dj?ïAà˜6?rûªoҎ>?Yëà³'Ë?=N"=?–%.çÜN?rFè•×Ío?ïç"ô¤W?ZY~Ík¨M?B¢£tž?:
¹!Wg=?cÓDK戸?V»Ñ'-ck?゙iÉ.?ƒяÈi?Q·?c'Ð?c,²ªB¬?|Š`ü¥²?=ð@d]?ïCXŽ?&?'Tñ¤?l*•úۂb?v´Ñz#ç?"â, ëõ?¼TR¿Iê?îCu
C$î?Ž(G‹žž?m:ÏXžà?U)¾8Œä?©õh=•³?d%ή"ÍAGN4FGL J0433.7-5725¿ïӟJMÀDvŽÞT´À:Š:ÏߦÄÀ<š©glö£@_]³d?úBfýe
?Àé(M&#€?ÐC†g­Ó@àÇÀôQv@Sn9œ?ïèC ¾¦ï¿Çq¾ß#fŒ¿Án+ALP'¿Üɘ$y‡¿âw3"«C¿ës,è–VïAGNbcu3FGL J0434.0-5726SUMSS J043344-572613?ïrÄÏc'0?…ÛQ«ás7?ƒR‰ëÜp?z
a|n¨ç?ø"Š'ó?w1—€Ób³?ï_Ï°¤D?'›°Å/À?k\ñ­i?qqO–Õ?¥J'r^?vºœs"¡?îX™ÆÝkù?›f©#É`?o>ɋÇ?–¨C•)h?—}ˆ_î#Ë?‹0¹ð˜?îŸü?}‰òLƒ$Y?{1‹'>·?^´é:È|?¢­	¸æeû?z³m'è%À?îAh¾ìu›? T¼øL
?ŸÝ"Šoç?•;V,q·?—õŒ¼rÇ?
l¤õÁƒ?íú¤Ù¾¢¾?³+MU?Š¥êà´
^?£F‰Ý¿V?©¬7®|†?ªû±?ìdèËÂ?§=4^4?±RãsI§(?¢ÕsÛâö?§¬^&Ø°?–ɨÁYðð?ìÊîvüÇÍ?–mzt×x?ˆa×cé.c?tHm.è?¶œQ\
G?•{HOîãAGN4FGL J0434.1-2014¿Þy^ðÀCzÞô¾À:>))ÄõhÀ<"VE†òÎ@&.iIð@4FY€¥?¾£eூº?ÆJL)y@f¨Þ°û@	éaþw¿ª¿ë¦œÒþ¿¼ÍfC½¿áLýpÇ¿éòB<»r1¿Ç^,»C¿ïÿùJYQAGNbll3FGL J0434.0-2010TXS 0431-203?ïà´ªZöµ?fáÑBߘ?Ré<Øðû?\4÷™é?eÖ·{隸?\>.÷I?ïЕ ªsË?VÓêÙî@?Bœöû t?^ëH"À?uaìv5?|j˜Ãü?ïr¬C%«?ƒ6NÚÒH¶?jYm<k¯?r³UÄ`ú7?Œè¹œ¬9(?îÞû¼?ïÏW»°µ?TZm&!'p?EIԔupM?2GB'‰%Q?uªçó5k™?R͏­H?ï­³Øñ.'?}%æ[û'¤?lL%$Ù$ˆ?oH@$Ï…?{ˆÈƒ?t'˜ö³ßl?ïWïPìgÙ?–—Ð®]ë?\²HM´ÜF?{™úþfŠg?"6ñ]ï­?'[ôZ§¹?îê(=µ˜?'ªtÜk"[?z¢øÕ¡­?7½Ueü?œ?Û}¸¿?Žp!Ôz»ê?ïy]*
Ö¾?sg2Á·?[ï©tÎ?O¨Sl Ô'?ŽF·'ª¡z?r|…KSÇAGN4FGL J0434.4-2342¿ãð*y?êÀCùáuÑ=À:{k*ñERÀ<ˆ]
ô@t/"î;@¼'Æ#?Â8MyZ‰ä?¸IàsȤŸ?óIxÔýó¶?ÿþGn(¨?Õ%‰&"Ï¿ã‡"ØaV¿æ·k;¸<ó¿ã6_mMá4¿æ:®â¬/¿ðAGNbll3FGL J0434.4-2341PMN J0434-2342?ï±8'[0?vÝÎË'LÊ?NÐ9<֓?BMã¨iÛ?ÄÛÔ·ß?uZ\Àfâ3?ïm7Ÿî6C?ˆÄ—ôþÅ?hî°Z1?nÖH°Jƅ?Žvlc€¼?ƒ¨¾Ís!s?ïpN6;H?wÿø¹³Â?j€¾á7¢?h¶*¾)z?XÌT>â?ržpÄ:cr?ï–ŽÄ Ñ?r&€ôe
?IçøWs?\ꍄ7ߢ?•´aF?m!o«zgÞ?ïS0µÓó?ˆ,)6²¢?^Æ"Ö5y?P弖I‡ ?"­}ˆ'J?‡?";K?îaß
¼òd?ž€AåÅņ?{ajã׋?€%qKk<%?¦uáú¢Y?šó§6¡c?î™Æ2?‡vÚ ÷'/?w7[^'ø?n¾ÁšŠG|?œA1;žY?"3Õ>f:B?톌Û)?-LAâ?"óŒ%¯?y"
éÎrb?­ºËÏi
?‰}ô˜/ñ'AGN4FGL J0434.7+0922? ‰KœVÀ8ñ|å-íÀ9—b=⹞À<ˆv[¦ð@ RGS?þ9¬CÀI1?¶¤u7d›?­-rð³*?ös?wåë@0»O÷º?îÄâÞ0¿ä/P…S'x¿Ø,¹¼¤¶ƒ¿Þ0{rçÿ¿Þ\ÐERD›¿áÜP=Z(•AGNbll3FGL J0434.6+0921TXS 0431+092?ïøO!{OØ?@	5ÎY:4?Ü¥ ?Ü{?Þý]~?K‡æ0žÃ?>kBA6·½?ïå¢Û{€?iô"F~"?5²Ž1_ß?C'µ€þ"†?g¦ÒðXê;?fO­À©À?ï·ÑÿwÖ?t )sn¶?RÞíÿ~þ?>v:˜<ì?_D¦¨–Ò?sÍDËoØ;?ïswË=¬?f:GQøl?U¤{<9Ö¶?3CR÷ðŠÓ?B‰Wü?e…wv¼è?ïô(m Xª?HuõÀy4?*½zµœS©?랛³ú#?TWv)ï?F_¤€g?ïª{n‹Mü?ƒ.J0â ?DŠ‹ò<.©?RÛ~HãJ?"{T«?':Ž€e³?ïšæPµÞ?vJZyð<?Z‹³†6†Á?W]˜NýQm?…ôõfÈ+À?têåqHi"?î"(w~¢Ù?ƒSˆ¡ýPÛ?iògrtKŠ?QCFó¤½è?¥.R Â3?'Ê™'y¼AGN4FGL J0435.4-2623?êßÇÓóvÀD6ä:§›»À;OÞÉN"À<³fZOØ@¼{päš@!G®zá?Ê-ªɏV¿'³Í;Kta?Åû€ÿÄÆÄ@xsŒ>½*?ë¸[#*?îì1¡¸¡ó¿àµpà<ì¿æû½¥h¿Û¯ùWoRž¿åQ‹
ÜAGNbcu1RXS J043518.7-262120?ïÚùƄÎ?aôIeg…?B^_Ñ<Ö?8€èªµ¤l?p7¢û5t?`ÆóiЛg?ïÐ=Cµu?p<C©Ç?A&I•Üŀ?E>:Ÿò+?u¼•N¹¶?mq—@|³Œ?ïPTÛh_Õ?|‡‹ŠBP?k8aŎˆ?oÓª"eB½?'Žb(Ë™?}Ðé
žÖ!?ïµÇxò?`ÐZõÍ]?XÔ'ؤ
?D
­
ŽiR?T=züùÐ?^»Ôè?ï±EÁ;…M?w¡äq?WòµUil?OuV§?€°9"8?uN5sN‰)?ï_u.US?ÉšÃY>\?YÀ²1Êä$?m6"£Tò?''f5äÊb?ŒšÖ
Eì?îÖô¸›‰Ö?ŠÃc/uï?t›ôÖiÎ7?téœ@†ç?Ÿúk½ÿ"¤?‡§wû$©!?ï?g(¦?|Ü6ƒ"Œ?jl ¥í?_¶ßsm2ý?"ÏJB¨Íè?z˜âËJñ]AGN4FGL J0436.2-0038¿Î)Ö'¿aªÀ>›Ã?…QÀ;«ÆÂǐÀ<¤Zk†`Ø@¯}óJå×?þ"þ)f*×?ÒZžý0ÂÁ?Üÿf<Ÿîr@êf}ãZ®@'§Dýàì?É»…õLô?܉uʇx/?Ë| 7 ¿ä',ëp¿æÌÁd8å¿ïöBmbÚAGNbcuNVSS J043614-003637?ïÑ®5)yî?bîˀk¨?R¹g•'…H?G%ò3Vg?rz‹'nˋ?`&€1e–?ïq.õr²?†x£ËcБ?jÎRízz?nk+l÷A?¿
^œÊ?¢
Èø–?ï=¬UUi`?†
À¶.žÑ?x™ø‰õÿÏ?vܛ¨cË$?'#÷+5
?ZIÒMìz?îœÚ–0zé?|òÞÈ
ã?'ÓG—-?e'-¸Ç…?¡qÒÒ¶¡?xݺ#àv?¼ó™s?tuE1y}ý?k!`@ë)E?`´-î¢&?Iø­'ÿ?p¸êz,Jò?îIvoY:j?¤‰¾äˆµ?H†®'š?HZ{]õ?§wZ'c>? ‹œ"ê›?îÀã®?'`º2žìG?ƒœ²Eg‰@?ÌXêÖ?ž/Cœ?Œ‰'ÖÕæÜ?ìÞ—H G?•4Ú%›ˆ?Ž¯ÏêM6?zÀŒo¶?µOJsÙ¦?"…G‡fßAGN4FGL J0436.7-7148?¼"éñºGÀAûÇ£˜ À:ÇĹ­À<‰‡¿}@ð¥¦Ã"Õ@úR¹á7¾?Ä1?¾
†?¡J=CŠø?ÜYÀ@Lv@¬ó±³?ïö!úü‹¿ãë½RÜF¿åòCŸ'Æ¿Û ë™á¿é\,9
ä¿ähF&*AGNbcuPKS 0437-719?îE_$þ'?ľ€"÷?¥'
û™"o?Ãñôžæq?Š
ØÔ ‰?ž}iôK¨?兩êÓÚ?x»nx,Y?W¨OáJ¢?X
u=¡{?ƒœ»]žÌ ?u^K;E
?ïj^Éöÿ?|›ü}›—?f/¯Ò¦?aR˜0"o?Üa­S'¡?y¿–ÿn‰?ï\Ñö"€â?jŠ½ýLç?n᥺¢ÈS?JV® À×?‰Œu­¸?iš{æ?îâ;Ñ^Ï;?°êÁ {ˆ}?ŽT•U'©Ü?°Û`ÁgG?"Ž;.¹­´?ŒÔˆ_¹^?îú²Õ™"Ô?"VÚR'‡\?dŽ'hs¸?h:÷SUÎ?žÓƒO?'>±¦'?ï$ØLÄ?†Döo¬Œñ?q~ðüüó?klElÖv?›:Oje=?"4‹2»ë?î*âIê7t?"êóÄ×a±?…¹Ú6°d?i–'@ J?§ãdßjß?"¨nˆG,AGN4FGL J0436.8-5223¿ì;_&¬ÀDºëp&ÉÀ;x¶ËÈÀ<¤FvÜÖ@+}‹Q@Þ0å{|?Á҅ÉX#-¿³­FàH?ðÆB‰èK®@
¬Tš.‡¿åCªåx,¿ë‡—Ù¥ù#¿å>™=~:ÿãx^Kò¿ïy4i"P¿ïúâm©QAGNbcuAT20G J043652-521639?ïû1WÍ·?Cы¤{>?/[­–Iڟ?0«s]³ ?6ÇleÒ
¨?>æîåñÖ¸?ïÏÍ:Zï»?vxZ!dÓ?Ets[³F?T×ÊԒz?ujÔs+*?sã•f§?ïpÿÙ֏?‹Ü¡þƒX?VÁÃ;mX?_ä©ã=Òs?t"Ž&G?ŠÐê}\®?ïéØoS† ?HÇՌyù~?<N¬ÈBp?(1ÿðäáS?b»>¾Wm?F¬^Úiù?ïõDÜí›?V,;‹\0?H¬HŸÒ?H¬|)W }?BÝüS Cü?N>ƒòÏjx?ïgáV$W?'/ #ÿs?X³©ä`)p?jJóöae?'xš™¿qT?ŽgD °œ?ïCr4i®?'Îaó2d?]-–¹Yñ@?e²ß(T;?›D¸Qü³+?'}<¤Ÿ?ï´Dò'?n{yÁ¬Ó?ZµÑžó¿Ž?QqFÛ
?0c"BÚ?jð›ù»+[AGN4FGL J0437.2-5846¿¸|8`0ѶÀDØ@žUÁÀ;:†—DÀ<—7£|g@ûy¹h@`V#ùŒ?ÇÝÌ#""z¿š¡éŸ@x?Ñõ몦?ý›Eìu?áŒwr¿ét ά Ý¿ìx¨B~՞¿È§ùÈ-¿éoîo´Ã¿ïü–ž½oãAGNbcuPKS 0435-587?ïÍshâË?pF7°½?SəÐè?J§¨'Ù?t'	Sì‰Q?lí2Ú³b?ÏüÆÔ?"~2Óy/?bcìn<Ær?j¿®Ô°Æ-?†½PèV¿J?€óe=øƒ<?îØ'oj?"—X¨‹ð|?tËÂ-.?xTÌH%•?Ÿùº¾ØX?'L9!¹Ø?ïŒòPâ=?k8Ýø\]O?fˀã:…Œ?OË¥`Uö~?‡‹'¹¾b?h:ÛB,ª?ïSÀ؈ÿ?‡'«­§Ê?eA݋-?\,!*KõÎ?ŠG?TŠ¹?…,̜?îã
Wá'*?Ÿžç¼[HM?pylÚ÷v?}ÂU/Ff"?Ÿ€YÒeZP?šÁFäÜ\?îDRkmó_?™†v¶œˆ?y|vÔ%?yáÔ>î??¨‹X÷¤w?˜ƒ·Ð©_¼?î{Y_?Gö1÷©,?…û"eœ×?yqï¦|Ö?¢Ñ
¿ ]?‰ù`
7Ê<AGN4FGL J0437.4-6155¿äþ@ątÀC§´ÃÁ‹PÀ:ÄC͵*À<¿	A=@ŠŠ}òÊ@>aÝj©Â?ĕpªä?¸± Hõ½1?òÊɽMÓÈ?ý÷børÿîWZ$8Äm?ȵ˜¾'m'¿âJ¹—e⳿ä5V#"Cø¿à| 9›Ø¿ïþb¦¾EKAGNbcuPMN J0437-6157?ïÍËoª‡Ó?e'Ó±!Þh?HÙĆrƒ?:ƒ%_]Ú?uÿ³ù"?cÌ*?`"s?ï‹xüb‰?Í¦UXÕ?\îÎ~¤‡÷?`*¼–´Ë?‰ƒçPÀ?Aæ"Šú?ïo˨¤?y~(ó;èä?iN4à?Aö?eìŒDlL¢?åmÊ·2'?tò¾}"·?ïQŽ??ÓL?pÅ÷Uju?t`]˨®Œ?WÚщS]?¶ ¢‡µß?kçŒ+Êñš?狼^E¹%?tÖþòi…?[ñÎї1?Lš-mÔ?ƒsJ5yÃ?sܓÇÑ?î¶Y‹ë
Þ? ¢5‹²c0?pm$›•È?t­Ì°3W?¢—¹)¢å?ŸY\õ&ó?ï
rؘ:§?"Ö²_ÖWÐ?s=.…ã¨?m1\"u'?™âYHh?'^Aâ ?îFÑuo?ŠB@YwÆ?‡_$éônà?sG†\¿j?¥Æy°÷Ø_?‡û\‰4bAGN4FGL J0438.4-1254¿èH'™šñ3ÀA£.3ðÀ:‡;ibš)À<^÷ÇLZL@»Ç<êìó@.O[‡æ?ÃÕgûè?¦ÏÆÁã?ävÓ xñX@p¾µ²ÔÔ?Éص¹4êm¿ä¨¿¨!¿èqÐý³õe¿Üv<eç¿ìÊkÞöE¿ïÿûÎBÓAGNfsrq3FGL J0438.3-1258PKS 0436-129?ïé)§nC€?\^ø'r?:ßᆡG?+×°*R­ƒ?c"|S)Ÿ?ZU—ÿ>"Ë?ïÛiÂ*KG?p¼a"Í[ƒ?8ªµ²·jŽ?C{õ㘘è?pÀsy$©5?nôlC¸ ?ï¼¹Š¶ãé?sϊé¾Ð)?U§½ÕSP)?J«¥KìÏ?|9K1øç°?rùS¼¶AU?ïÍP©¡à¡?RÿjWÜe¿?Hð{õHÅg?*Ä_Òtž?v9›Ð~#Ç?Qå"¢‡A?ïÛDy##é?f:m_b?E)0âÆE?: )î?¡>?oqBéƒÄ ?dR#K§"å?kU?‰&räΐ?K*ö¦u'1?Y†Öu·?‹`õÆ蝓?‡©dÔ<û?ïƒÀ'^$	?ù\Ý,"©?aH~	uh›?iÆ|L›*?Š½Ö«A
œ?€½"^4ÅÛ?ïubjƒVŒ?rsÛ¨µ{Ú?a}ÄÒރá?J‡R읅?ŽGô3¹­ñ?q-了"AGN4FGL J0438.7-3441¿â€úŸÕ8ÀD¦^5?|îÀ;"xt…äÀ<ãJ?¿2°@!(dC '?ûë÷j/HÃ?̈éH-–;?ºPÓZ?ð¦<åd@›‹9¬³¿ïù_‰X?ïúµ´)h?Ù®åRп½ÕçRµ­¿ïÿÐÐgŒ?ïÿ	àÔk¨AGNbcuSUMSS J043612-342230?ïä{
×÷?f˞‹[<a?L+p÷"ö?b.¢…iJ?d"g>6Ì7?Z•G–•?ïȋ
ÏU­?xòކÁü?Hs.¥#×?U'$0‡Äq?x¬$Ó¬·?táF–dHf?î̧¬"¶?"iE­¢ÿ¹?éeØv¢?"¯üé`ç?vW'ðK1?é¼¦÷Á'?ï–û1d&?mÒZ½}/?ViE
Ý*–?Cㅏ÷T?‡t‰¨
?k^úÏN
R?ïÕ¨Ö£eJ?jÕ<71Ó3?]©ö!ô‹G?a¬Ž&Ó
?k'.iÜÿÖ?dEýÈ:¿`?ïkÂÊ{Ÿð?n€4o}¤?[&Ë¥0Ú?rHt·"¶?ÕDþRO?‹Þ
rC?îqìj旓?•wÛ4+œ?'.(Ê}?"Áµ.¯ò ?¤U¯ HÝ°?'í4Pˆ'[?îøÓôÿ5?ˆúŽgf‹?fvÌÏ¡Ê]?bc³¡?žāh$?‡B!£îÑAGN4FGL J0438.9-4521?ì.â'&òÀDâ$ p¹À9N¾7ޓŸÀ<Nªaâs@¨ªÙ‡ñ@c¤G?¬™šròç?¯­Hß(*R?ÿ —Œ™@/&3E|·?ïþŽäÒ}¿ãþdßӏµ¿å}U¡E¿ç0§g¸uþ¿ç­ý~ÆY–¿Ù³œÅH'AGNbll3FGL J0438.8-4519PKS 0437-454?ïæGß+ç?e€çî?' ae_¥?ä0»Aco?h>ñ‰¡Õ?dòã¹*µ?ï¾@0WòÁ?}'¹sÂÕ?S·ÔDö·$?`;¼ð'ó?{ñòµ
˜?w[#…²?ï¢&Ý~9±?{ñ:pŽeb?X!öÜS4?]ª–ýC?"r	Ë|Œ?zq÷`–?u1}"?[ÉöX_[;?m‡¿™^év?Q~©¬øÎ3?rq"­Ï™?Rf|ÐÀ`?ïÂ-›?vdæ_I)?>î•f%¾l?5f¢ªÐ݊?} <…Ÿ?uìøI#ö¯?ï:EӖ7?–ŸIÕã¬?ew§ÆùQ?sbfmmyÕ?–Pª"?"[âR;?ï\Ì£v&?"ÈÝ"17˜?cv!r&>?^ŽÆhjý?'÷§hz—ë?"`9Ö	g?ïKSâ'?{'Uæ'?"ÔÄU‰ž?p
®ƒh?ˆVC1É&?qþËivÄ^AGN4FGL J0439.2+2151?وæ0ԑÆÀ0KL<µÀ:V3sÊÒøÀ;íK¿3@çښ?ܺ@¬Ì¤ˆàå?ÑÈ3'˜?à¥e¶™…@ql¤nò@X¶ÄLˋ?ïþ8µS3"¿ã¹]¯2³¿á6,!qé¿éò3¿ïúÝ¡†M¿ïÿR@>´qAGNbcuIERS B0435+217?î$…3Â5€?¡É¡QÒcB?rÉ=yœÊ?‹É4•G 4?©ZúrXK?žu863`?íÂSÑR1j?«zóü'‹ƒ? 4tf?.P0«)Ë?£ÎŽéž[ú?£HÅEãǸ?êµà2ksR?ª%Þ˜?­µÅ'r˜?™ñ1p\?»Å£‰m¸¦?¥Y¼Æø1?çà©V-¼¯?Ÿ§¢šÁ?³9Ï&}Ê?ŒS
F³vB?ÆàsA"?œJ×Òã<?ìä˜ùê?±CMŠka?šÕ³1b|?˜W"ñ¬-°?¸‹njü)/?­œ{™zü%?é¡ÞÕ

/?ÁýgXm™$?»¾"ªhì?»ê—Zq‡ú?·2yĤûœ?²'s‰Gc'?çæ(OCM÷?°PЁ¬?µ£Þ%–Æ?¢~ï3ö?ŕo±qZ>?ª(`¥¿ê'?Ý®C¢õ–x?«ò¸GC[?Â՟]—¤'?¥­ЃOP?Øæì®>—??­êjƒ¶Á8AGN4FGL J0439.4-3202?éH@AtОÀD_鞔«À:}WƒÀ<†"¢¹ÓÌ@ßeSÁÉ?þò?¸|³°?¼ÂSw rç?6¨ÈO~?Æh®ª¢ÖY@±÷ò"ò¿å@XëS '¿ÖByaÀºE¿ãÜ'"€{¿Ý k…˱¿ÎÌû›Â=ӿ䔦 h?ÚAGNbcu3FGL J0439.6-31591RXS J043931.4-320045?ïÜÞA¶¦?\½8ÝÒ?=ÞÊR¿;?*M2/~WÝ?oeäòƤ?[5k›QN*?ïÝ?CÀQÈ?p¬£k8`?7Ók¼;?CVÙ÷zP?oà¡Ö×û?m7ˆê/?ïzbì"Ab?z°NÃÎ?Xmwº::Ç??Vȝ‡˜?ŽY•õ) (?zL´¤çõU?ïÏmi̼?T	™Q5TÞ?9t]kã?"''RÆöó?v·³á'?S§Ãn de?ﲛnc"?t®}g›?Q5æx[8?AŽ!Z¬¸Â?2t8
"P?sKdÐ_¹"?M,iÒ?‰>5Ós"?B'Û¦Í_?O'Ç?µ­G?‰|"Ûç?ˆªŸ¨Õó?î÷ѱ]}?‰TJt‹?aEh®VøZ?PÉþkZ?žÝ"óY…V?ˆ­o'É–˜?ï҄áj'?q ¹:Í?O<×~'n?@Å[®F?Ž'FWàä?qBçãSùßAGN4FGL J0439.8-1859¿ï'Ø
Xê8ÀB¢\þޗÐÀ:
lâ˜À<L›ó-u@؉À]¨¨?ü*î «†?»"(k"Œ?¾Íç©òØ$@}¢™ó\@?'˜rÓ?ìÓ}c.¿¨Ç(H¦¿àÿV"tn¿Óeî[è´	¿ãó·‡Á*¿ßqoC"ºAGNbll3FGL J0439.9-18591SXPS J043949.5-190102?ïUgáÏ×?½Z°Ù.ãv?'b#äö40?½xö)3;?o†ÿã_ö?]E'2é@?ïŽÜ'³ŠB?ƒ"Å_Ë5¬?aÙÆB¤?cz½Ã=?‡Òm½ÌŽ?€Š ¶»?ïmžò|'U?|'ú0Ž
?b^PË{T?XPÙ#)?W'äp?{d¡Ñ´°§?î^Dë†:0?zä]ÏÌV?€oލ©N?_Kã3V3?¥ÿ¹§3¾§?y-¢ ƒ?ïqêwœ]ˆ?«±üèV?'` ƒ2™ï?«är3/?$Á†¸?ot<˜Œ?îȲµ/³]?œ'L(«"Œ?q*ú`I
?yizî?¡Oud)L	?™ðÞ¾«¬?îÄL8pgz?'aü·Z¦"?s®ÙÁ?qÁì»&÷"?¡EaRé!?Ž×ŠÏ^?ëÿt
؏è?"À¶2lê?'z¯…¢F?ysìãwñð?»e³è>1-?'A‰­ÖLAGN4FGL J0440.2-2458¿Úr€&Å«ÀC‡+À:ªá»qZ¶À<q¯x(/Ê@!²§'h˜?÷<Æúû´A?Æ-—<òú‰?ÆêÚÿÀj@_l&™Ç½@ßDd¢¿ïý;)¡¹ú?ïý¯žÐ?݃¾š?¿ö+ëÁ.´¿àÏìÝ
Œ°¿Ê¢Âiq‰AGNbll3FGL J0440.3-2500RBS 0570?ï»Ëd?"mØ;9Ð?JgŠÔo–?=]%àÖ²¬?3‰]'Í?"_?äC!m?ﻇnã|U?…C{"¿?QõüªÊM?[w/àæØ?}¾É\àj¶?'fSUñXÝ?ï팥?s9¼ú¡?h°™üCŸ?qˆ×*¤éa?šŒLœ>N??—=4C˜?îKî•õJD?ŠËUU&`?qlü'|¸?Wõœöڋ&?©'ß	H%?‰t¬
› –?ï…;§ÿl?…ùúþ"'?`-Ò<͌¢?Y'<¢x1?Š"¼‰4{ñ?"_`д¿¹?ï*Ù@SÀ?¤É›Åç×õ?h£"'>?‡[]#²L?—ghZa"?Ÿ8dãh÷d?îZ®@‰vÑ?˜d)g…ßÎ?pQ3s|ÓÖ?u)ÕRÐ*?¨Jõˆþ?˜ãÌa¥´?ì"xüò?¡ïEUq6ÿ?|aé®t¼ÿ?rž7·G¤?¹–!<ï'H?¢ªÄ½žAGN4FGL J0440.3-4333¿ï/"àCøÀDÆÙßÚƋÀ9¤*ߧšäÀ;åíùm@¦'€x`d@³õ€J=;?¹»æàõ"×?Úù\ã/å¡@C!°9ï@Â=Л
¿åEÄe>Š¿ÖNØ²´¿è™'6É?¿íM%'pˆ(¿ïÿ‰b"ʨ¿ç€VÂYQAGNfsrqPKS 0438-43?ì"—HuT?¹[GS,¡?½0GÎÿ5?¹,ÅðÖ?€××µc›?{»qå†f;?ïÎÿLÉ)?w߬yg³?L"
vâr?^ø>¸õñÞ?ubþºÌi?sF&ÑDj?åñn«'ž?³n»
†t?Îÿ""S?±u²é?²ufqבU? ÅõPÑ3!?ïËW¯	?bãe¦f?P	 Åõä?@¬ñKÅmã?vRÌÍ?`¸}‹žÁ?ë܉-ï/+?¶uK/¶L?¾½-FÎà?µñôt?'ôÛÖTJ?}WäC' 0?ïfY¿u1—?"¡d†jÒ?gcØÕ·2?{+Þ9`»?Sû"[MK?'νÂâ¡?æC_^Æp#?³¹SÂKžÍ?ͳ_0š°#?±kƒ'‹?²~F§MD(?¡Ž!½Ö??ï4¤Ô؁X?ˆ]?N´ù?pÁRô+Nû?e¯ "@?•;£ñt=?…ê>àÌAGN4FGL J0440.4+1440?àÞv,y}À4~=jΫÀ9ߨ‡s&À;³\ÜJ@;2ú(P@ÿV"tn?ÈÖMªñ?Æø´FÄ	°@;{Q^—?ýig…d?ï^"ð•(ò¿ä´ÔÞi,i¿Þù‰ƒÌÓ®¿å†D
K¿êGq®™¿ïþaAGNbcu3FGL J0440.3+1444TXS 0437+145?èþôl£í0?¹¶ß®."«?'½%¦1÷?ƒ-p" b4?É㖨M'ƒ?¹:†¡ŠÍÑ?îXzÌò.?£º:óÍÀÞ?•¸˜ëUZ?œÝ^¶ða?ŸDß^ò?—0NÒKõ?é	°ec5?­0f¨•/ß?¥ù°š—9?•»µŒåQ?ÆZýýqZ`?¬ŸZAͧ?æŠ\öâ0?œñª³º…Œ?¬í~`<²Œ?'j0W,'ù?Ð?;zæŒM?›yÆW¢?åÿP.Zu0?À%$îFM?¤ÖcP;¿?¯*·fB°þ?Ñf"9z—m?¾OI©Â0½?ë;ág—?¸ôÿdoXb?¯½°å"?¯.D4Xn?¶D¨Õ<!?°ÒÜñ³0?äҏùv'È?³Á…ÿ…r?²ždc6?¡¾S9óG´?ѳ<³9¨Ã?±âdÎ܋?܎l~ƒ
?¥AlPÉÆ?¶°NÀA?•˜U<k—Þ?ÝíçКrï?¥ƒ©RŸ4MIXED4FGL J0440.8+2749¿ï7ì.֛òÀ(n~¥øL­À9x
†Ñ?ùÀ;éò‰õ·¨@ $~Pg÷`?ÿU0cu^?¸ÞÎWˆ?¸ç÷±¡@Ⱥáè½Ä@6ù8¶¿æ£ùdo¿àTl~Xu¿ã…‡"ݘ¿ÚÀWVP¿Ù²¾c}}Ú¿ëÃßóðþAGNbll3FGL J0440.8+2751B2 0437+27B?£²ïx?|0%NÓ~–?\r"|	J?N[ÌǺ ?ŠŒ"†'¨¡?zž~?ïSõÍp?—䬙Næ°?pÖÍ09Η?zæ‡üš?'K"ÅCN?"¹Ñ NÆ?îuSýƒ#?"äkÑýg?"6NIzÏ?'ÏÔNVfG?£šW-ßo?òÍÅù§?ë¾Ë.Q?"–9ªÖß?'ô_Gj ?s'ö¨	<H?½b)w¿÷t?"1ìèõB$?îûÍõR
O?"à÷g…>?tkÄғœ?e?"å×Â?›ky]ªy=?Št3úA?í¯Ó
>é?µú–W©?'O<S,?£<´Á\9?«ÛMÃÀž?°Ü©[% ?íBWy ? ŸÙKK²û?'d>°³Ê?‰Žì`s¯»?²æ0˜?8ZJµl?å¼Õ'±—4?¬zÒ&ã¹?¦F¼ï2s?'*æ—))?ѽ~ù×?«³V¨/AGN4FGL J0441.3-2617?îÚôœŽZeÀCÅ'U°6À;ù>U¦$ÂÀ<ý/iz@"_Ë1í
	?ø…ÇŠm¬¬?×ýÍáéO?Ân³|n»u?êG-ñªÒ§@|±¬_ð?ïÅF%~>Ê¿ïç7a–
?èìcÔ¿àùþ"ï6¿˜¨[ÜÓ2Ë¿Ò`UÀ¦Î¶AGNbcu1RXS J044120.5-261659?ï±çÛ÷–?ˆL\yþt?8ÔCv©?E/,MUwØ?'¿—ÀàŠ6?‡T#²{š?ï‹ÀIþô	?˜' ãË"?am2¸Úì'?jŸ%sNС?ˆ´ Å­ª»?—d¯ÒÍ	6?îœ"g€d6?"Ÿ¬ƒ+C%?X]Ϥz–?^%zMüõ£?¥zë
¦ë?"ˆ–"…º?ïf{jë—y?w"ò¿Fp?/ÿ&Vó!Y?$ã:<†?'ð"R1ûü?vþÞÆߢ?ï`™âƒ‡"?ÎwFÞa?Iÿ;Ò;ó?DOCÿP?"Ç0â"6?³ã2Dä?ï-ß·56?Ï]bì\?dx£´x±?vüýJzÃÝ?›+/¬ß0?šàÕ®¢ß ?í©Îâóø?Ÿý•/-"?]
^ÿCu?fQ+á™.X?²=_kêA¤?ŸÁÃë"W?îñ6Ó@?—ô€RÈ:F?8¼ýyö??ä!èù?®œØ¯­Lí?—æµóAGN4FGL J0441.5+1505?åkj°‰0|À4	ü›ÇqÀ:RžŸ'×ÞÀ;ð³£¼@!ÔE¼ø™@<êòQÁ"?Á™#RŸÊ?vX\ÇÝù?¸]†Ð&?ýòº‡¥Ñ5?î]'"ƒ¹¿ÚF\»lӿ七Ÿ\Q:¿ã—d53¾s¿×ü}"€U%¿àìm|]]AGNbll1RXS J044127.8+150455?îŽZI*I?ÍMó[Š?d0´2ä;?VÞD#/æ?¥×P&'—Ë?"'iÓ?SÉøÿ?7M	£5Ý?dÚK¥Øò?pz>R՞°?‰é%ôWí?ŒµzL Å?îöK?™ƒ4ю•"?uÜ6à±m
?myê×k¹?¬%j"ç?˜²ƒ—Æýø?ëÞã
"pñ?–TO¦ë}?ÇØIO±?eÍÝn´¬X?¾Ïì£$?–|@dÁm?ípÎuÞg?¨xe"ÊËí?w²îõÀ†?iž-š1?²þkRÏÔÁ?§»œ´?îÄ|®ž±?¦Çô§°~P?wS9ÆDÒ?†*òŽÄ? Ü͛SÙ?¤Çõˆ¾ç?ëâ'Šçà?¨2k´šV!?ÐHÃ@nŸ?w«šH{?¾´ºæðî?§…üõ,¿?å6
W˜?­ö€½d+?•¶c®ïúÌ?†TøƒHš?Ô8_ª,d?®¬–FDAGN4FGL J0442.6-0017¿èu#:;À<v\=îxÀ7æ#ú±À;¦$p!Ñ@4{;4´h@ßýç!é?•@†Êñ?±¯=oÍ@ÃÀ;ÄÒ-@¢…pµȿÓc?ò©€¿ãYø™Ú¿æ\Ëè¡>ª¿æ••"z›¨¿ê¡Ù¿#–Þ¿ïþš¥2TAGNfsrq3FGL J0442.6-0017PKS 0440-00?ïØ8œ¡?dÜD[qT?Yð
‰Ö?M–û¢'Ӟ?kpiŒ›
[?ai¿`LvÉ?ïßÙÀ-á?qû?:ûA?7Ö4¨=?DDÁ¸õ?mÿk™ÏÊ?qR׺zÞm?ïœA¼Z[8?"ß÷˜›¡?eZ&ìżë?qÛ.".ø?ƒ™:>dÊ?'~|;«H?ïúN ýÚ?0(¨'ö/N?!1Óï$?Ž¿_?C¬»–?,R€Ïފ®?ï"#_Ö?ru"ù͉?aŠ%}
Ü?Vè9ŽÞë?†›­ê
T«?€'7d`ËÉ?ï¥ãòXL?b(q'#?Rä.7%Ô!?jlñ8õ'}?"*}0È5?ê"£7	ÿ?ï|ñBM?Š‡÷˜˜áº?g	í>V^?s³"¡ 6W?‹4(=Æ;?ˆÊ¥±ÿ?ïòB3‹?N»øƒs?3îˆ:³?*ýCY¶•Ï?V÷…ªÈÅ?KA"kí¤óAGN4FGL J0442.7+6142¿éë¢i»Ÿ@$^°ËæÀ:2"ѼsÀ<:ÏߦÄ%@ ö}¼ÄA?ÿÀ©"£˜÷?¸F x[Š¿u-¤Òîá?¾¢8FîQ?ú"êpvµ"?âÈ9À.¿®¾NÀézê¿çf>ù:!¿ØïõÆÁ¿Ý"F¡$'}¿Ö¨À(#¶AGNbllGB6 J0442+6140?í4P+]ô?²'ƒ˜?iÀ…Jfy?['u>3­?µzze8ù?±íPEà?磳u°'È?Ÿ亡žm?ŒE±«'Q?i,V"£?Ϭ×HP?ÅS· s[?îO^E
Xâ?•R¤¢7[?wS'þ1|¯?s°>"ïʀ?¨«NÊSÑ?"q«:—/Ñ?ìÑSòÆ[š?i½k­c€?"+8&²ÓD?sèóáÅH?´j'_²zä?·›3ãâ?êMèsã?¼Xótƕ?{Å|i©÷?m'ç=yý¯?Åê3£N+æ?¼ß,™Õ?àÖ:+Ao?ÊE"£1â•?—¾î³iˆâ? ôøeÜò˜?ÞRd Wgµ?É«£</±?ìWãC†½t?¢'.Oëòú?Üw[ýê?v"À߶5ë?»dT#©ä?¡Ü_ÿÔgõ?ç>´‰ñ>?¥¦¹£áWZ?¬<	ö—Ú#?"&þDò?Ëö+Y¹É?§ ƒÎÄ-HAGN4FGL J0443.3-6652¿ÆŒ›l¶WÀBš-û¹À:@èþ[»À<t>ÿðÈ@û>¥,J@'Œ¢:R?½PÓs?¼f7íW1?ü°qgKh´@
ëc€­åV?ïúŸmîðä¿æ¸à0×¹¿äƒ`½Z¿æ=ø=éŁ¿èè®	"&¹¿ïÿÿ&¦³AGNbcuPMN J0443-6651?ï¨@^{?³Ä…ô~Ë?9(øþ²ËE?+ÁKrú3?…/è&ϵ{?³Æ•Åe?ïÖdĶäê?s¥«'p¤U?Aõ6°½ ?K"å «"?rŽöÂÝgQ?q_)À÷Œ(?B"	?kúp
J?Y²r¼‰«^?G´>ï²eW?"`ú
?~þw&›V?ïÄ?1ïo?Yܽû4©?]U·Ž?|ü?:϶~^>?vŠùª•?WN˕~?ïÂȂmáŽ?z3þ;¨?S/L%ÌÞ
?Q™Þ9
W?yÏëÅaµ?w+!îɖ?ïƒø7Öþ?ˆÐ_f]{2?P$´Š?[4Ýg,?9½Yõç9?‡Oäªö'?ïc0¿"?†]âyÖ\x?i€Á¼d~?hüV½zï?iæKï"Â?"ÛÃ@Ï+‹?ïXñÅnxr?v#lãÔ(?sÿ҈0?Y™5$å?Ãÿ	:/_?så}i¹CAGN4FGL J0443.4-4152?ÙÉjF¼¬ÀD{BB…À:ôG1ùAÀ<±æõlÿ@ €ö|²Ã?û…‹Z;µ¹?Ènþ"n\?¿"xuœ9?öÑPüDŠ@'°f·š?â=Œ²­è?Üæ´yý¿â©ö©L¿ÀÉljÁà5¿ã»aÕÝ퇿ߪÛá<ÆZAGNbll1RXS J044328.4-415151?ïã}<Z"
?pïŠÎºâŽ?6Õ	¿¾?E4#«¿Ë?i¨"`䄗?lÌâáª&?ï¾Xtz2?ví"Û´µ—?LϪk'å?QoaiSå?}9Ð_l4Ñ?t7Ô^çÄ?ï‹M‹¤
'?s¨¢D9Ë?\'|®ïǚ?\"›Ñ$9?‰§­…>*Ï?r‡Ç??ï7²æ5˜W?nE ~&U?qA"`ñ?R7òg=ŠP?"¹bÑuAå?lc A¶$0?ï˸÷> ³?gûàdoó?I~I2ª‡?=»`±û?vó»@á×?e«ºT	w?ï6Gíªgó?'ç0@ޙ2?`g,_³‡•?d)ÐMÕ´Ê?—*·…b·?³×¼J°?ï@÷'
ºL?™ ï´k?aŸÏ¿Iš;?R=ýµL¦j?•­ÍFÅ6?~
J}9?îÍäÇ7?‰‡^;q0Ÿ?í—²3¥f?naنø
?©ÃM5&£9?ˆ.²Åå|òAGN4FGL J0444.5+0719¿Ðù·Ç,#õÀ7ô§Å¬GÀ:W«(7V®À<"O¶
é@¼R˜©.¸@yŸâÚU?ÂVy^e»ò¿›àûF̆ñ?×>;"»f@	úõÕÓ¿¿þëWýB¿çÒ(¡‰Òý¿ëeHŸ5Û¿ÕñŠ;­«¿ïÿñAÌ(7?ïý ¿¨¡õAGNbcuPMN J0444+0717?ïðŠ6¥.?Rúȓñ$?FÊä»u¯ê?@:«ŠÔû?T{y&iA©?JFф¤A?ïчYñÓ?{Æô\½?Dæhžô`?O{"ó©·G?tŸ¤:$p¥?y|nµ?ï'_ pð¥?€sûfÉ{Ê?`û8n©$€?dm°€˜?‡)IÐX{? ­YFòž?ïÝћ­^â?V1ËødÞ?=ˆb?àG­?(¿Ò–‰'$?n}X
dÄß?T™ŠË`"'?ïÞàø 1±?e;_¡V–?XÊٯ홥?S…Ägߞ?d¹šCRî?_Œuֆ3?ïyFŸ:‡)?–G6ïW¬?Wèb78?vq&Â7?Ž±K÷V6Ž?•Sè+ð@<?ï­'õ»ƒ?NÐEóÂ??i±;Nó®?h¬P9Ÿ?™T&?QF?‹äêSZ?ï‹àK–4?x•Þ"ag?[¡Œ±A"•?P¢•$—Ÿ{?‰"˦ˆT?wø®YD—AGN4FGL J0444.6+3425¿¸ÆO±ÎWÀmtO]5eÀ9Ÿ¤¦=À;¸Ï-Ðã@à²;Qæ@™ÐcZBl?¼5ŽäÒ?­ê4"ö?óÙ&­ó"@M£ÔfÊ¿»j^˜'±Ä¿Ò£®Zñ¾¿å^ü_ag¿Ü^î7€ŸÎ¿è,	æ~O¿ä»ÁŒ§ÄAGNbcu3FGL J0444.5+3425B2 0441+34?ïMrλ?®cçﳙ¯?qºb[¦¯+?¬€ ê¿ÓŸ?›‡Ä[Ä^Û?˜­¢?íݦ6?°¹Dv'Þˆ?S¾BÂ-ž?^ø­g`:?·'£¿]?°†éë/ª?îÖDFo¿Å?Ž"ˆy[?qW*e"–4?h'ì‰#'i? pÖJݛg?‹Ù¤Ñ¥‡?îQò¡ų?wÄ匴b?yž&"'än?RÚãë"9'?§­?çÀ?vRÓI"'?헷I™Ò?ªmE^Ì®?p¹u\A'(?èÜeÉ?²6°7J,?©Iýó1ü­?ç"5%jŒ€?Á9"ýAE?cÎViãg?s»Mà¾à;?бù·V?Áè<}?í'j /J?£ÂSL?'¼ô¯OO?y¦OZ¿<ä?µÖ+ßÀ?¢yÝÉk»²?볬À<ñx?'wÂMO»•?'bè5;©­?py3o.',?¾	ßðɉÕ?8'åWAGN4FGL J0445.1-6012?ï"©LPLÀClX£/D'À:£ó}:¾BÀ<®þs8@ìVò8Â?ÿFŽ¾?Âæ¹G‰×Z?¸`ÏΉæH?õ>.‰€Fâ@	lY夊?ï›h zÉË¿êÑùÝQ)h¿ÙJM@¥Œ—¿ß£ü>Ty¿àŠÕ±wÝ¿çÕøÅyAGNfsrq3FGL J0444.6-6012PMN J0444-6014?ïù«E…y?;<³QLys?tàqÑi?Å8FI|c?Fb`žÀ?8ÀíÄ£%×?ïÚò/e{ã?lèN?¡~1?7ŠMEø®?@ؘÖìì?qCš ‰?j<POÞn?ï¹4Üxñ?k¦8.e?P<§'°ï?V-¨í	û?VgÝã4=?h"s	g~?ïÒsSE­?Psa/çm?DS(Xï?&teSåû?t6l¿0?OÒÄئd?ïóÀ ³X ?N®ªj?*íG®^l?Ÿ÷c'Üg?U!6cp?Lœ@ƒy?ï‹Ä¡Q–B?"·uNk÷?JóՍÿõ?WVªMõ@?‹_¦ç\†n?ƒk××$d?ïÓ•FL?¬ð
ö?S"¬'4À?B÷Féx?&Å#¦œc?~ôHb¬‰í?ïƒTù‹±?ncƒVðU?W-G¾?CiÈ>^z?ŒJ[ðv4?mè7½ÑpAGN4FGL J0447.2-2539?ê4z8³ÙÀBÖ5"_õÀ:ØøúRAÀ<¨!S6Þ¹@Øée´»@>ª¢ÖY>?Àh‰@ÛèI¿©ÒçÃô*?êÇ5žd?õ'¡Æ
ëÑ¿àôÈý¿Î(•µßJ~¿æהܛvé¿Þ)–|XÁ¿ÞµñäíU¿ÔÖ[[	fAGNbcu3FGL J0447.1-25402MASS J04472149-2539302?ï½|¾='?w¯ D@:E?Ev
©Ëk?9 ÍíT4?~'ß‹V?w"Ñ)¿?ï"Pÿ÷Çw?"fŠÛ1?\ú¸x"?_¼Š­iw?‡LhðK°l?}¹Ář:?ïM{'ŒMð?…VÓDC?jg7Ç®?k×rÍBå?" Éû?ƒŠfÍËğ?ï1 NU?t/JÂå?r;çöí‡U?V¾>'Еa?•N¢–s?soœÃä&¡?ï‹+¨áq[?"¨i=|?Tïfbß?H€¨¢be?Š—(õz³?"$·ÏlŸ?îÔq©2
a?š¾Á÷P?k%¹ÔË¿t?qš(XŽ_r?¡‰Ï$ª?˜F‹'‹W?îÚìy6±?Žçâaesî?q›"%Pnp?mxrth? ÅâȘ¨?Œ¦F÷3Ü?í—Õ/¾?'iÃD=c?ŠWõUF?xü	3,³?¯ù5XÎä"?œï滑AGN4FGL J0447.4-2747¿Üˆ¥	S)·ÀCbäѦÀ<SxM¸À="—jpÐ@ßÀ‹@ÓM"îê?Ø«¿Á¡u†?ïô%Á°Žÿ@Ð=0ã@
òi™ÌšM?î}I׺f™¿ítw Gô
?Û
Ú¤{Ë¿ëžñݨg=¿ïíØë¿[¿ï PØ_¨AGNbcuMRC 0445-278?ïí=ñ??°'"Tìt?r½®©ý'$?‹f ¼Ü;k?˜ì³öPÐ?¬pŽ8´Ê?ìÙ~ïÒ¾Ý?¸{_ƒq"À?¥ ÆælA?­Êä
ô(E?¬ÇJèí¥ñ?¬
ª$¢?ê˪ŒÕ'?«`ä·É1A?«Þàb…?ž´6ˆLá?»³;xžn¸?¦''ô'ME?î)®!ƒú?•×ã`Ÿî?£&üÍ~J?©°¥ë/»?"|BJò$r?ˆt&ÞüŠ?í¤lgÌì?¹ÕJRg3ž?‡s¢i?íR?˜u6Œ#Ò?¯ÜPèï¥ç?¶ÿm@DZµ?èa_?øàÉ?Èïß1ºsj?º§ÐuñN?ÂŽM¶R?Á&šÅ#ò4?»4°¶Áš?è¶h^ÊL?µ0º'n¤d?°R:©Vø?£a8Î)y?Å@‹>?²Cw½R®?êå«ã?¢?³Æp¨ü¼h?»0KÚ@u?ªŽèJ2§h?³øCSÁçú?ªÄ¡UáÅAGN4FGL J0448.6-1632?ÄÅu—© îÀA8:}ªOÊÀ9mÆÚD""À<OËn@/=ƒC@ò?ýq½¥è\?±]!™,â?­r¡L%@!
 ë2@aTåµ{ø?ïØRÂD³Ž¿Ê¥ªžú'¿à+ÄÿÎ׿¿Û6QØ7¿Új©Ø«þ¿à­#^ÔÌ¡AGNbll3FGL J0448.6-1632RBS 0589?ïÜ8d—ѐ?aMÇñâ),?7r¯NÔzÉ?(¿úLŸ$?pl¢©"f‹?`p+Õ<þ?ïÏfîÝ©û?u€Ç,¦."?DuO_Ýì¨?Mb¯‹ÉÙ!?u½Þ±¸"?s"!¸Ÿ?õƒz?uvwwþ
Õ?[b8Yº½Ë?\¤Ø$ac¾?…ŒÅÖ% ?rìLRi³f?ï$Ze¯ºÌ?o±bMÓùŒ?l›f—w?JÛÊIˆÐ.?—áFƒ&x€?m'ºz`Sˆ?ï°M,6G?w8Æ&á²_?P×LšÒb?Dg
üîp*?ßC'`+æ?u†®–:r?ïn\à3d?‹:E€zª9?W8xTk
g?bÅo
ér?ÀÜmm…ƒ?ˆæcÕE÷?ïMCÛ6û?†''Sñ?fad^Mb?hQ]X‰M®?"‹pÙSeO?"˜Pæ™Ê?îÅs+	³?ˆMÉ@ä[?Õ[V¹Z?cɚ_+#?«©û­?†ˆ1¾½äAGN4FGL J0449.1+1121?ÞâÝN"ûÀ4¼«Oœ À8-e•†¢À;'·îvï@¶Ä¼2ã@ewS?¡âއ	t?ÁÇ­¾"¥¿@©qÁ
{ê@À×õŸÔǿјº¡|¿ámm "Êþ¿çga8)<¿ç¿]¾L+}¿ì§%pÔ)¿ðAGNfsrq3FGL J0449.0+1121PKS 0446+11?ï¨å¸1Æ?ƒªíŠúÕ?i>	´{Ä?gx9œ·?~îx¶¥
?V|;Jf?ï¡Æ
b`•?Žà1È=à¥?euDþ÷<?sø"0æ:?'IŸ\¯^ú?‡,Ɨ',?ïVâîÞUÇ?ÂݓL+/?%=³1Ä?…÷ rAD?‰"¡@P?ŠRéÒ©÷?ï‰!ÓJ¦~?m£…uGš?v­…ªfî?`,(VÓ"?'`ÈPëò®?c_j3#'²?ïRV-?‡»·RqyÛ?påÜ@Ç?lwÓ$Å|?‡¸û0MÕÀ?"v"2±Àó?ï7šmvr?¢ìŒfÈdr?}ÿ|ë$/?'¥Òš¾ž?˜Y(ъ•¨?ž[˜r¡3÷?îæoÜ ™?™z¼¸W;?Ð‡²àiA?'i´P^z$?"Tn,³†8?'ÃXø8?îÝP?ÞgT?†åì4oi?ŒÌè°Àî?y­(¦'
?•ïƒ¦«4~?~"ÂJ(÷RAGN4FGL J0449.2+6329?—ýÈôú@'Ía€M˜9À9']Šõ'À;¬Ê‹¨?@ԂTƒí@íhžO?ªÐNâf<?·AªoT̋@Cf½Ë¨@C4ò% ÷¿Ú%a#""¿Ó**@Ejm¿á³hãh­¿ä¡÷ÁÃu¿åÎÀWs"\¿æž£Ä•ÇAGNfsrqS4 0444+63?ïì!å>D?R¸V¬ò?2hÛMö¨–?"6F´Ü[?a"Š¹›?QàÑÚ²Lq?ïßÙ{J½Ø?tÖáXÎO?=pÒõp?J/6"'c•?ltä§3´?sc®V¸?ï@¡Õaé?Ž	.÷Â?t`çÜÕ¦ä?yRY
RªJ?'Ó£Ç&-?ˆ{æÛ_Å_?ïãÝò±ZM?N§øN̒?2¾_ǃxá?K°"a?iÊAHÉï4?MâW4ÿ»)?ïÚÁâ/ð?g'CJ©±?:/\B¯Õ¬?/:YÝ?pü9¹"t?f´üNU/«?ï­ÁÖçÙ?†¸–^ý?Wî³îVÐ?uþ€Ç‹Ó?'ùÉÑa?‹®0­[?îðÌ	?'S>=à?wà$Ũµ?vö¯À"«³?›îvC&¾?Ž•µÚæî?ï­q9®?pyßH´&ž?Ma7ˆØä?;fى²?'Íž3%T?pE

AGN4FGL J0449.4-4350¿êœáçTýÀCõâŽÕñÀ6ä˒:*À:À>ð֗Q@vµú£IÇ?ûþÛ<Òf?'¯­|r?¯­DË@Ö"Ì«?@Lêt'š?ʜ­	ãل¿Ó¥"EO@¿ÜA¤ÕÍ¿×ÅP׈èq¿á*½]Äu¿ÚôZƒGsAGNbll3FGL J0449.4-4350PKS 0447-439?ïà'dÜò?ep¹Ó
?GÙ •›ã?F'qGËo?iâS¹'äË?bøZZ+ì?ﯽôS	Î?ù†čo?P"~]aÞ?Yy¼›Ý"Á?þÝٚ%?ŽïœöêYZ?ìâLeU¼—?©­¹¯`@¸?Û9óÙ»?ž{ß' ?µ2:
¥¬Ž?§¡È"â]s?îß8¡Ôs?ˆ, 5ÙÅr?\hÄ®&Ê?Geå"»ê?¡)/¼?½®?‡º46û:?ï»Myì'I?t¬g]¤y[?Qößàò¾å?KóvI˂Å?}ۋ!Hßt?rïZö+¤ù?ï6FX–Ö? äN
hÄ?fõŽ¬'…?{
Áÿ?–t݀+çî?Êˆ‡ N?íW›Tå
?¨No"zŠz?€áÔí<äÏ?‡fÌÝ¥?³&èv´WÚ?§DâCgÅ?íèõöá?›Zƒ
£ó?gÇW°?t?WúdLÀ(ù?¯ô0˜=ó?šÓU´֎AGN4FGL J0449.6-8100?½ôç0–À?cà·õ¥À;À´%tÀ<ží$[)@ êÿ	àÔl@¦@×`¥?Ãþa"Õ<]¿½n¤ÁÁ?ù›ÞM'Ðÿ@*¸¡Çx?ïÿ¡ÁnT¿ïˆ_µr=4?Òed®¿ïõYÀÌä¿îO²
¤Ÿ?ïüV'TàAGNfsrqPKS 0454-81?íÃܲ£<?·FêyâÃO?jálY)û?€}n|ì\?±
€ëwÞ?¶x,XðÔ`?ï;¿ o?™Ÿ	'ü?vÿɨåp?"\	¥¢?'È*YMÇ?']7`
ùû?ëø_ޞ?¥æ…v:H?Ø¯¹SŽÁ?Ÿ5"º?¼		$?¥J"Nð·?íáú¨Ê†n?›àªx"¹?míüù_"Ï?ct‰†¨X€?°ºÒ-Ǫ?›Êÿ†ø?ìÉü9´2?¿²Uò¶Ÿ?"hIp±uÞ?¡Ó	²\?·#©Dù?½©#òV'?î4{ ¡z?­öîF_®é?‰8U-šG2?©]Š^c?¨¢þCӚ?¥Y½3R¯?êöÕÙÞ$°?«­ú}ÝÃ?ŽíцS ?%ؽ×ø‹?Â5Ë~n?ªZ†tª ?çÇ#Ø¢C?¸ñ(ªKÌ?Š§³öÂ?''"8÷ÞÂ?Ï9|§›e?¸¶…ŒÂ&ÉAGN4FGL J0449.6+3027¿ßîýy=ÀÀ"GýœÀ:4žÝ¦8äÀ;¸sQ0t<@	=-.@¬œ[ùŒ?Í/5wÜ?É9(Ö
b?þË|j´ª@å¨îÌ&	?ïßG"Ô@_¿å%èâ­â¿ë@óæ¿âW'X\¸h¿ïéÄ¿¸T¿æ$AÓ´óAGNbcuMG2 J044950+3026?èø'Û£î÷?¿¦(àž?'…('?‡)úVF(p?Éíì–ýÄ?¾¶uUm?ç£Ï»>¯é?äN¼ím?‹'^¿'?Œ'+Ø ò?Ï·«2HQ¨?ÃœÅü¤?êð ÖS"+?¦£ÙëA£?  œ?'œPö[Ÿ?À=THÏ?£Í¯è
æ‹?ì}+¾?'¸Y¶Qè?'¾ÖE¯?mþNÞ}?·¦ì‰г?'vÈÀ?ú?áÂÑÝi
q?Å©¨
-mª?¢XÓ-s‡Š?œ§¡°n'?Ú/AÞ¿
?Å+«3¨'?ànE뜛­?˛ßHv?Ÿ	°Ì{?¬êþ¤±?Ý2âLÞ!€?ÊÄb>¨K'?ä"‡î,?³!â%jõ?µJŽ'Çí€?£$µtŸå?Җ5Pﱩ?°F -™'?çz¸­Ûñ?§®I†µ%?¦Þ»ÔÛN?‰Wuoo?Îbn_ª?§'DÅ/^7AGN4FGL J0450.3-4419¿ÓüL»´:tÀCáþ!ÙnœÀ9z:э%îÀ;¶íª'æ!@\‡à‰˜@I©|e¬,?¶9Ô1;·?¸}BöÊ¢%?ûÕv¿yþ@æ}"¨¿×XÝ|Gy;¿äÓI¨Pí¿êŸ¾vÈ´9¿é–ß?–¿ìs§A¢â™¿îW…BI¦'AGNbcuPMN J0450-4418?ïöêËc)?F`aŽÈ[?4Ǔa¾r?,t…ÚÈe?JG§Ä˜?Bdì‡"‹?ïÙ¼Ð3X?v7F?ç?=ÌdZιc?Hˆéjó;¥?qDѾ­à?u ¡qœ?ï{³èâò?"* P·¹?o"úJ?t9ä¯öŸ?‰.vF>Ží?"leÖë?ïÇ9qø?ZÙñîXY|?MQQ¦Å·ê?3ýÝÊ-?xÍÕ«®?XrŒmÝ5?ïï‰h|žÀ?WöUiak?DZçcTáZ?@ÈVë÷9?V¿»%ŠE?SÁ7ïå¾|?ï{9J3?'þ·«}qÆ?TÊÚ°ð`@?hÿ	œÉ?Ž˜R2,?™¯q¥½G?ï&6"1º?¿Ý{Ó?u³—kqá?zuµ½}UÁ?•ÐsO¡áŽ?ŠÿÖ¸©—M?ïgÌRð?yq3g—.&?gߐÿÔ¥?XÆÿ‡Ïâ•?¦ÆA²?vŸZóÉj]AGN4FGL J0450.4+7230?ì.qK-7@1x¢Ûa»À;µ'm,À<¦µ™ª@ê«5ÎC@Å+M‹¤?ÆölXmÕF?­‹RY?ãIþ†ƒ<`@¿̀ø?ï¢S².»Õ?ïä>ÙY£
¿ãÕµ¿'¿å&ÜÛ±¿í¬=Æþ?ԁHŸ¬RAGNbcu3FGL J0451.6+7231NVSS J045109+723014?ïM%6:?¡‡>{¥c?pX±Ê£_?yaÒ»Û?'7†­m[Ú?œ¡,%´¯?ïəK^?y΋¡…âˆ?Q6·Þ?Y®Øôb
?v咋qY}?u7²ã†f?ï<-ûj?Öóœc[A?xšÙ¹½?}tXâP?–'ô‰pD?‰f±$Ã?ﯲÿµò?dþä``?n¢Eã*±€?VìzD·Õ?xÕ]%I}?\o–'¬'Î?î­Pžå0?¢é¡Oãœ?íÿ‡•!C?}`©YÉSª? ¯v2ˆÔ«? 9»'?ïc>ÀHôª?'dÏæçÏ?fV`•/<Z?tRðûCÅ_?Í[ÜØZ5?íŠŸ/Œ?î{{Á
ô,?•Š…Q8‰?'%rËç"?'ºŠØœ÷?£¾ç@r_9?'g:gS"?ï/Î6ћ?€âW˳e?'sòމ٢?r.j"zù)?äŒÊÚØ?w'jºÆ<AGN4FGL J0450.7-4938?Ô2z)'tÀCÉúëÄÙÀ;Pûð¦Æ©À<ßþŽæ¸0@¬áUoô@>µÛ¿ê?ųZµÙ[¿–©@€£©h?ÐëÙ!ÄËÌ@Y¶o"5Ò?ï|š…Qãø¿ç8~–ÞÔ6¿àžvþdŽ¿äZ^»w9ó¿éÀ:SÜ?¢{•w öAGNbcuAT20G J045102-493626?ïÁ©RÊ'V?kûVs7XÔ?S.súëU?CúMŽÖ?z_¹Ë~ž5?iLtõÇ½?ï©áC??•º'åâ?VzŸ±sC†?]Éj…'T?'¸[E\ë½?z ®ž©òÚ?ïa¦ïÝ7?}:—è«ÛÕ?g@+¦2?`¨Aqt?x?õe°#—á?{# æ¹`Ë?ïÁjú°ñá?XwLh•>?SZò_óv€?6¦û½:e?zsÆ-Õ­?V¯yÎwŨ?ïTÉòìŠò?†UÅO#å?j.»øé´-?^²+9«?' ê$YM:?"–šÇÓ$?ï)HM»d?'0þpJû-?a5uŽ¿¤Z?m'¸´{Þ?˜¸è<µ€?²HßdK{?îê%vkí?‰¼N'n³æ?t&«IŸ"F?s&x¡éª—?±´@Ú}Ê?†·Y¶KF?ï.$Ù(OÕ?zp[òîï<?kè	L°‹ç?X»ÔlªSu?–¾c«à"à?z6^òÖ_AGN4FGL J0451.8-4651?ÄÎå>;W£ÀCÀe¾ ºÀ9ßõ}ÅþÀ<A©n*@ü3öQ«n@ÿ#¶?¼¸ì"x?¹ªiJœ[k?ú|±|nX@¥CžNl¿æ‡¸Æ…Šï¿ã!'fw-^¿ç(èÁõÙ6¿ÝÉ%8HÇ¿ïþ˜÷³*d¿ïù|´†…AGNfsrqPKS 0450-469?ïõª$ü\?G†÷uI°?-;öÀ3éœ? ×//¥*Ž?Q8©æ?E™6`õ‰?ïæåˆ
2Ì?l2>(ø!Z?3V."™öö?D+ÅÕ."—?f¯²4n^?hÉOË}a?ﺷÜz¿º?vë½5R?`Î	¯‹?h–þI
z?z˜*¶9pæ?r–³Š'a±?ïôôý /S?:œ4d¶$d?)®˜ðÇÚ4?ÿRto?Rà2Î:?9ØG€p—?ïîoÙEšÙ?RZê@×ßÆ?=@:•@±.?10"Vä?[Ð>''âÚ?Pš	àK¾?ï¼9T	—ƒ?õºË·?BMšHè[?Tð—aðݼ?™¢¹`ï?€å:;Ä?ïm¼ØK?rîJ{[?lÑ{Dü(?v¦†ÙwÑÛ?"°M#ðK?x[NÎxØ?ï⶯7+?ZBh@?e
?BÓ8íÖ;L?8ù³¼OE?h"'.G(ò?Wd;S{GAGN4FGL J0451.8+5721?î$Y §¢=@ £úLaØbÀ:ã9º5ñTÀ<{‡(}Î@!³§ú/†€?øR7y…?Ó4ÖÁ˜;K?ØCP·¨xZ@óݗö+k@¡vÈ3_ÿ¿ÐO¯j¼6}¿ïÿèþ†®/?ïý›6QË¥¿Ôný?¿Ò÷si"(¿ë°Ú=x±mAGNbcu3FGL J0451.7+5722NVSS J045148+572139?êÈþ'}×­?¿û
?ýyœ?c`tá0¸?X2܁6Ռ?σâ‰]È?¿åÓÞ'×Ï?èÀ¸E<†T?Çw…{2.?{cÕ{ìÕ?"…RJ?Ì"COh§?ƙêfÕf?띖c"3×?«	ڑ‰ê?{ËhF?yÐîKŸ?À«K2XlÔ?«ý1RU?î!±¥ëÉ?Š÷Ø*'?e~šŸ/?Tò8"M‹8?¬ŒüØ-¿?‰©R6h"Ò?äIÕ+ŒÔ?ÈWqÅ®å?s''`_§3?mypQÊ>§?×
¸ÑÔZ?ÈT/¦¥Š'?â[±!~2"?Êÿ­yM?†å¾lT"?'«wCa?ڑoɼw?ʃn8[ªå?çN5ì\Ea?³ƒ¬+ôN?…y4Eî&?'nn6ƒ8ž?зʄü‡-?³‡‰Çu'?ë_G³ÈÄÕ?¥j'!G?qtýVý?k–+Ȫ,?ÁúeˆPC?¤ÿʲ§ÿAGN4FGL J0452.0+2100¿ê<Z']À,ø§ayWÀ;YzŒŽ\À<…ñÓ'é@"³Öe|Üu?ùQÉ÷/væ?Ï+=…òrÏ?¿!%¿'6|?òkÓyq@sœ§Àù°¿îÂÉ.4¿î²;QæM?ïÿXÛch…?ÝÇ×DŸí¿ã¥u«?q7k¸FFAGNbcu1RXS J045214.8+210307?ï6¢~ùú?³iUÏʖ?Q?ULÚñ?lhKíaj?˜Ì$ª[?²¡Jj†?ïk:@m®Y?¦Sjø?U"Ù&K?ht¤Œý¬ü?'@j[ñöÛ?¥É®Îù¼‰?ï)ŒÛ	?É',½îÑ?V·}®ý'?V>d†;¿±?œÒjˆ™s?Kv§Ð_?îk?¾~LÙ?'zàD?PQWµú"M?C©Ôa"Ÿº?¨ÉyVê-Â?'b–çÒP‰?ïmÔl(r:?§_—]\Û?G'GH¤?Zµ…G"	‡?'‰eî-3?¦•µ­x(?îÞû;Ü5\?°¥˜Ém¥S?`ÇÇÎ00?yϺ‹TN
?¡ÛtãàB?°‹,̦W?îƒz."ë?"ô{-k?]1ž|?]ƒ`Òݙ?¦ßkŽXÐ?"Ô¨êXÛ?뾍™R™L?«ŠÎâ'$?fØüÊX5Ç?iu±!;Š(?Àªe¨Àö?«¬Y	9AGN4FGL J0453.1-2806¿î-¼§CXùÀB"Â	$lÀ8'Îï¼»ÞÀ<©@։å@A|wð@P­Í-DÝ?£¡?Ö.ËE?¸ªÀ³cð@¼Ý!®¦q@ùÃOöb¿ÖE»ámÛ¿äêB‹@¿èô¾þØㆿê"úÞ­õÇ¿ëù÷2ú(¿ïÿÓÀíAGNfsrq3FGL J0453.2-2808PKS 0451-28?ïì¹nB 0?U¿¯¯âý?N
‰bEø?G*U¦½ž?WŠš©rØ?L/2½P?ïÐaé÷Lu?v(FXCü?D"ßHª™N?Má°Îø?u<oˆiÆ?t¸ô'è5?ïrÏ$ê?ŠãØD3½?u"Ï'œJ?¨€'ZÊj?ˆ³d³î5|?…r"*©ÿ?ï÷0[žŽ?5ä	9eЭ?8ϳšz?$>ævr$?G8,9Ÿ0Ù?/?t.Fnþ?ïÚÍ—ª?h,ƒ.†Å¾?UÙeö£?Ni«ˆÂÙ!?jF0ð¤]?cž‰qô1?ïˆÑà)mY?'VZœÝ£?Y£}È«ž‹?kâ½D®I?Š—F.Ü?'²u4iÑñ?ï4Àì;Iz?'þ¾dé´p?{61kßý?&¬ÿµQæ?'šV7WÆ?pٍΪà?ïéêg<z/?V7%?±o?OnŽg@?DM'A¦¢?\sê²_¾ú?N`÷l]~AGN4FGL J0453.1+6322¿Õڂö9á@(V|ᛑÀ:S±E‡ÊÀ<+¯BxJ"@ ¦ˆgB.@zlãX)?ÁJº"üq?›-¹ÌƒÁ?Ýú$Á‡@émÇXÅ?í£J¨š¾¿çðÇþ±Ì@¿èú)(î6¿ÑËaè¨K¿ä!æ­j1¿à@"°%ÍAGNbll3FGL J0453.2+6321NVSS J045312+632117?ï…ŽAC9?·i:ÎvÐ?S»;îG?C‹<5Ž?šÝ…¤ƒÓ?·n>txj?îÊn?<šª?¥v–•pN£?c,"¬Ø¶?iWçÔ?¢&YßYJ?¤ÃX»Ë 9?ïNÐuMßÝ?ƒ¨5ߥ‡?cÇK¦@ë?b$Ñ:z?"­囈"?'©êŒJ
?îãŒ{ñ4ƒ?~éðòH?pUæuB1á?Q4lO,Ü?ŸxöÜ¡ÉA?~º[
sWO?î¬B$ƒg?«¦t›ÎÌ-?b÷•_7œô?b¬x0ú²?¤dcî=?«L6ì%?í-|Q#"?¶ø;m¯Ôñ?p•‹ù­?yèðôë§?µ"ôb{&?¶Žàx	Ù?îe–ëœú*?—ßdüoVï?rÁ§å©?qÂÉ/Á~?§N\HD+B?–L'›±i?ìpÇ¸2X?˜æ-ÍÁß÷?Š×¢fùˆ?t(RJuÓ?¹!
íñŽ?™yºi
ƒÎAGN4FGL J0455.7-4617?é"o'*"zÀCi˜áõ²À9
¥ÿ©þÀ;ðšrÝm.@&¢†}20@ÝÓ4ÅÚj?§!­¤¾e×?´âÎì·£Æ@	ÿG¶@yX«gÍ¿¿ì 	·¿ä±Ö;áWž¿ç¥c¯˜	¿çWìPÓ¿èŒYÙ¿çƒO
)N®AGNfsrq3FGL J0455.7-4617PKS 0454-46?ïù;÷ì¤ó?I'{äjì?.KX×$D?G7KMl?CŒŽTßk?5Z¿÷e6à?ï姏%¢Q?küö2'?µ?4†#£é°?@ˆo6"?gÇ®
¯þU?ii"Đ%?ï­\¹î?vü÷d¶p
?[üªÍÌ7?W{I/õj?)xùêN?uÉS‰G?ïí"
"1?ATÕÍþ!?>Q'îV—?#{_KÃC?]S—¿•Oà?>(`:ì܈?ïóºI½cM?I#`µ€?3	AÝ­Ð?(6¾Ê'ñT?SÉ&IGÌ?F¬bCøðp?ï°qgKh´?ƒ7Œu¥Ó?QZV¢H÷?l:‰}g•Ù?³ºîX+É?a1_Q×?ïzA"Q*a?'a¶CÁ?gD$Ϛ•ï?gÞeƒkõ'?‹ž•ºŽr#?€:'Au®?ïÎЀ"­?a†Bü֊?UÙÎ'ÁÁ%?BØCaÍO'?s!L9Â)?^2"¯£+tAGN4FGL J0456.2+2702?ë0´Ö`õ8À$0H@áÀ9µ~q'
À; Œ‰ޚ@•tÁrüw@ïÇ£˜ ?¼xtŸ¨ì?Æ.ëzâÊ:@£É%x_@ phó´m?çÜ"N‰{¿Ü^d¤ÅFÇ¿ãc3vO¶¿æu
þÆD¿èå@6&¿ïÿ¯b® èAGNbcu3FGL J0456.3+2702MG2 J045613+2702?îÑÈùÈG?²U¨¶¿†?wހKèR?Ä0mýC?¥Ç£E©}?°oÔ¹=>s?bH¨?§2dzTº)?Uô؇Â?bÈõÌ#E\?¦63«™šr?¦†`âÛçN?îÛ&)4½?'PiёÌ?wàå‡%!?vs'ûÛù?ž£z¾?ô;6óî5?îË3hž`9?wˆ ¸Ëþ?påxRìã?Pìr˜o–E?¡0nÔ¯?u¿•Ìñbì?î(=¦ 2?«­…vÜ\5?·;•ß?…Œµ1c?©VÝkÝG?©0|ËK6?ìf<Gâu^?½FÒw[¬?qªý?Í¡
ú:(?»¼# /d5?¼4ì¥D.?î­EÀK?›Z,?yÁ?‰
«MñÜn?†Vàó††?¨qÀÍ<ß?—J2У ?ì¯uѓ[?"{ã},?ˆ=–»"=]?mX¤\šM‡?·|žž&¡H?"û"BAGN4FGL J0456.3-1634¿ä"bÐäÀ@^JÀ:Ý'nâlÀ<›×5Ü@ÎFtƒ‹?ü½úºpª?Ð
]O¼V?Òrsºâ¿}@‹G&/>²@ÃU¶ÀÆÚ?チ_æðe¿Þ51e'Ìù¿Û§Î›Ya¿Ó)<ÅS¿èÙÊÁÚ«]¿áœ]=ó«‰AGNbcuNVSS J045618-163552?ï®ô±\Ð?q-4&ßN?bySLÞù?S‹ó}¸õ?|j¼èÐM?m8ßûօ?ï`÷Š¡À@?Ž,_ŸñÏ?j'úE&âÚ?fîNoFA?¯c{©?‹—óxÉo"?ï`'`m±'?'šL»{0ð?pkË7ÝÎ?sUz["éð?¥Âg†0?}ÇM³Dl?îWüΝ1?zðÝ2€œÒ?1nnÿ·?aS³ä?¦3×~ô«"?x}oýËë¤?ïXïÃ
J?€£#–í¿?w?Ÿ'²¼q?g‡*™˜?Ž$p›3?{åc""PÅ?î=ŠמH?§yÖ8cý3?€þÉéªhs?……Ýþ7X?§ç¬®b?¥1ËÁ>a*?îí­0F¼?‹Î`åaÞ?}G*åõ{a?}ÕjÑí4'?›
Ÿ§"üš?"Á0ŠK?붉?•}f?•r4|"·H?'cê[	-T?|ø}[Ÿ?½ò»o"qó?"dNMؖAGN4FGL J0456.4-4043?ï•4•¼rëÀC:-ƒÆÉ~À;oºzº±AÀ<ËÆ+ÈÛ§@úu.«9)@ü!ƒÞFr?ÅEÅÇtô¿±Tÿ5Õ¥?élґ1ì@ý½Èäá¿å3!€nÅ¿ìé ¹³ë¿ÞžOv_Ø®¿ÚMõÏ¥¿êkŒÞl²?ËÞ3<ˆ]AGNbcuPMN J0456-4041?ïéx'Œ|?g\û°ù?4‡¦¾8Ú?/[ìýGuÏ?doVR.ºj?f"pƒuhÖ?ïЍ(>"í?t2PŸôŒ?A?¡)ßjó?H€õ5H"?u'wÁ"…?r
¾‰S³?ï;:šŸlÜ?Ž‹BL֝?ffä`sO†?t0ˆT?•ËÐpE'?(Ùê¡ÜÐ?ïìSF4Rÿ?GkŒ¢|Å°?&÷­fü™?"ªáqL!?b=>¿£W?FðºÉê0?ïÄî0—?xÒgKº?Km;=™[$?D8ÛÝÎg?z@MMÓ?vß®'Ì?ï…ZB¡?ŠG£þX}H?K?an¢Ý~‡?ŒîXó/"?ˆœ,ÆÝt?îÀ'Ó+¥?"ßXV'~?i†°¾BZ?vOð»Ä†?¢_lïá
?"è4ãƒ?ﻥDj	«?krÝ)&?BÛ~kÂÓ?6r¦%£òN?Ñ½?j¯.s‰NCAGN4FGL J0456.6-3136?á 5!ŸâßÀB‹;BÌ-kÀ9×Þuk¼çÀ<}'Õ1@êÅÝð@¥qŽ¸•?´8=´›É?µ8æÒÝ]?ùô3xÓPu@Q/¹¬²?×Îÿ¬óéq¿á­w!t™Û¿çøÃ*Œ›"¿æm¾ÌeŸ¿ê½ÁÆßM¿ïÿ°_ïÉAGNfsrq3FGL J0456.3-3131PMN J0456-3135?ïÝ®vAó?dÅ'ƒ{ñÐ?K =X|ß±?@k<«¶J?kizOâS?b>òÀš?ï¸CŠ»§®?Ós<àŽ?TîÒ-yRÚ?`ãÁñ%–m?~¢†ŽÄm?zAܪΒÐ?Cá‰Ñ?|°·5y?`fx»'i?dÅõÜ%[_?ƒø(˜•G?z[$ƒ?ï¾ìýnÖ"?[ÍU3'A?n½¦¨¨B?Q˜©1 ?q*®?P¸3˜m›?ï¢nö
'\?{uƒ¯q>?b{ƒ¦§?W¡ž_vê?'Åa¢H"?wâäx|sÝ?ï²(ܘ?›s¦ítu
?p:Šr»°"?­zÚ¹5?›Bµi?—/Ɖj?ï2)*ð?»çÍ.F?o²¨áñ"5?qė|d{¿?•È¥Ã
v?Š"ÓiŸ?ïV¦C–¥?z÷Ä @?"õËí«sõ?p=Áñ˜Ya?…`¯ÈN½?m"/ø‡»AGN4FGL J0457.0+0646¿àq0wt´;À5«Þ灃ùÀ:­¸4TÀ<ùÅS[È@/©RtA@¯U!š"?Á­‹¾åƒ}?ºF6mÐ=?ô—'ML¹í@ç~­Úï$?åïB]r¡Þ¿ÜK"]xB¿æ韀äA¿éå.X•¿éO€pÓ¨¿ïþcèݤ‹AGNfsrq3FGL J0457.0+06434C +06.21?<ØÎc?»¶rݹ?b£'—#?')®öî?‰ڿԗ?·ŒóÜWŔ?ïç閠Û?i¸Œ¯îs?2$GÄx(??'u½ëpÖ?f¬4WÕ?f@v%ÂÐ~?ï¨éÄ1ü/?v¥¢‡nÍ?^cè˜<p?`—~=EüQ?ó'y݈§?sÙOú*´M?ï̬›ÔÝ=?T·7båw?IŠ"lSÓK?)(MŽ—Ÿ§?vx_vØÛk?Rá~`\Nô?﹌¦*?©77AœO?VTZÆ´8?|jèÑòã?}å#@
û?¥æ46oQ?ﳄ¤"õE?…"Õdm_K?JÕãȤ
—?\Qa/9Z?qxžd?ƒùmü ?ïcët$6?€šP¡I»‡?m±zԖ?lŽ°¼_ê?˜Äe'Ր?|°ˆR…B$?ïl¥-Ìl?t8`§´1D?a™ö÷›¿þ?H¹®2;B?J~î'{?s:
‡AGN4FGL J0457.0-2324¿éVXÔNîÀAs;÷'À6q%»{k±À:øu/@­!­ú¤¡@ξú|2?€a—Ó#‡?³YéA¢@*x®I#`@ ȋ÷o¬¿Æ律4ë¿ß3âÂ\†¿ä~!nÑ¿ã¥cœ‡Š£¿ç{4ßZÃñ¿é@|ÇÑ»IAGNFSRQ3FGL J0457.0-2324PKS 0454-234?ïÐ@'.ß?mÇgOœ?B«ÁHæ÷ç??"Kç·ú?uŠ?_ï…[?kóÀ¬Ï ?ï7VbÒ?²ã۳ϸ«?q½¦3›æã?Ž;"	Aÿ?™)´
\p?±ƒÄBç;?ï´uVÝ÷?—ªfSB³‰?‹ÄñûÊ*?UªV€?V?†øXöú
?'–ö}Ձ?ïɛvs¥?n)_Fí±?V"©›ïÞ?Q÷Ñ?u©ÈËì>5?g´ú¼y¹?ï"NqI'?†>uö@'|?N!'ç(ò?IÝÍøªo"?‰WªAú¤¶?…É]¸Š#?º¼Ì?±u&f©Õ?{m™Fq®5?ŽlÈٌÊ?£¹Ì«Dõ?°¡"0f?ï2p"fEs?–'€?~¤Þ•m?†©º—ù®?'éùý^D?'©ð,bŒ?ïv7¿´áI?…Ô/[|k?gCÄ»‡[N?fŒÌ®™??Œ¡ݶ‹	?ƒHVƒ3ïxAGN4FGL J0458.0+1152?ïWF"Ó¥ôÀ2¦šíV°À:îê'ò#À<R1Xg @!ǎàV?ýÛRUÆÜ?̈́`¢W-c?™8 °d?¾žœ7ً!@-TÔî"X¿È¬Ãœã%¿ëÁ!h/"B¿ëÍÌsáy?Òó½‰bë¿á‡¦RÁ¿ÎÿùŸé"ÚAGNbcuNVSS J045804+115142?ï'Rü.í²?ˆÙWÅoÓ{?5¾ìfjèz?*ûØÇ$Q?Ž½I‰ý=…?ˆ¤ÒxVž?ï¼h|æN?'Ö¾CMO?M¾áb+—Å?Zíx›c?~å³5*?çÿEý‡?îÆ[$z?"wg<:ž?].^Ÿ_Â?W–«Kw$?¢°Ú¿-ñ¹?"d‰D÷P»?îùÖY­4?'üå磄S?XÙú™L	s?HžT»M©?ŸO%ÙÚ?'¾)ºq9?ï#žÊIÔy?"-9NIFí?E¡JVÃ{?A¦t
Þ#?šßaˆÑ¸?"çq¼übK?ïEO>?¢ÂôzÉqd?a^±¡°6è?s‹0¬ze?•0i)dRe?¢_FO"G"?í²Bmó®? C'MØ?d;¼BÌ?d?¿€W'	?±Ì´>Y¯? L"?ì¹}–g? \"¯ß*?v¡~‡Eâ>?rO¹y`ý?¸Éÿó•¹e? HœãcÈAGN4FGL J0459.4+1921?ïÔ5ŸcÍÀ, æ)•$ÀÀ;"ù÷¨À<BŠgÍn³@!ë‹Ô´ù@!Mø±W&?ÎM/Ége?‰régÉN#?À&¯X‡@l5%Ñ¡¿µ@cÖ>;?Û7½;_QŸ¿î˜Ù`ð?ßgk^Å"¿Õ;ˈ).Í¿å@¿ã°>AGNbcu1RXS J045931.5+192242?îÜCã.¸û?£ÆjŽtb?HÈ"˜3?JVý]Á?¡ÛB­	õ?£—È•ýÐ?ïÍ+'ˆ‹Þ?››×W,q)?2Š¨âóZ?CHÈs/MO?xJý½?›"4µ8?îJχ?é4Á<?]=Ãbž?[2é.}Ò?®ÆRÒcNT?ßٍÞ!?ï¹È)¾¯?iƒõªi[?=‹ñ˜&þ?0pà·Oȉ?€¡–
iuš?iBå˜m?îyV´}ܶ?©¬në<›ß?R/¾ÑºÜÛ?O¶è¶…üˆ?§ÙÁ"]»?©x¢—óf?¬"Àc?˜ÿÔ-‹¡?Jø…0_"Ú?fâ
" ò?ˆ¯Œ'×K±?–Ùz…,O>?ìúZ Ï1Æ?£Ü¼"Qxq?ibM÷µ{É?q2'õ½¤?·b‹Ø‰ñ?£«Ÿy¯"Ö?ï,[9{e–?‰‹wÂÚ/·?\ÃòUÃç?\SlAáf?˜¨Y«×?ˆïÑ߆8AGN4FGL J0500.1+5447¿ïùúÙ̀@'r%·I®À:žÆ3¡îÀ<,©ã"¸¯@Ƃe n@±Âþñ´?Înø†9?À±½½:]Ÿ?í=Àgc¼@Y9Ô1<¿ïÊô Pm?ïºiúÊ¿èín˜dt?²òpËD7¿ïÿø]ˆò?ïþ÷ýÖÛAGNbcuGB6 J0459+5441?èýo¼rÙß?È'q¾´0I?›Å½`‰‡È?ž¦'Pzñ?ȑ‰aµt
?DZäÿs" ?ìã£(—+‰?¹–³ä1µ?xt¶‡?ˆãmëCo?·`þɼO'?¸)R ~¿?ëÍ;8ªe?¤™
z|?" -%‹?Ž"»]†q?¼®äÑȬy?¢›ûI'C?îÑè'4¬k?…*Óa+"?{dÍÊr…?fÁÎabs¥?žéæ#ú?ƒ÷D*ãj?ä9'peÌ@?ÉëÕ{?® @YÒì?¬¡ô\,?Ó¸óùÑ?ÈMI'ގ?èž`	U?ÈuS/88?‡Î´B7>"?—9®Ëâ}?Ì
Ã=O?dzIMÑÅ?çžS²Qí?¯$­¡rÝÁ?œ‹="çÜ{?Ÿ'Wz?ÍõI…Q…{?®'ýÉ4Šù?ì°~°p\?¢{¨8‹R?"·³"ž`†?%z™ìS?µQß%"äÿ?ŸÝã&ì®AGN4FGL J0500.2+5237?¿–a°
Q@fL¡™B\À9ÖI°M:EÀ<ïH!×Á@!\$˜Ö¸?þŒý"$½?³ÇÝ_þ(¡¿'¸îª_å?߅&šôb"@-Ÿ¿ÛÓCÁð?ïò¥­Û¿è]¶Šk¿Ý– 7˜s¿×^ÎA–ù+¿ËŸ¥aÎÒAGNbcu3FGL J0500.3+5237GB6 J0500+5238?î'{[.é'?žÁàÈrÄ?g4&"S'ø?Wæ¢Za6-?¬çê…P?ø#C¥;ü?ëãÎ
†ä?ºž=å‹,?lޗ"'°?vÍÍgÏ4˜?¿úšó-V?¹âÏ­ý©¹?íÀWWb?–é»"â?y$GÝ\?r¢v›‰ß?°kƒƒW?•'tñ"cl?îD¥×5?"Óì
[¡Ý?…–­"ç÷ø?h1ڝ	ۊ?¦XÚL<C¨?ƒðôfõ"›?êë*Y߉,?µT†bI?€	&ê¯q¬?vÓ«ZV£©?ÃRÄ*^–?´ÇDx…â?å"ÿ}'ì›?È¡IL¹d?|ÑQƒå¯?ŠB™±8k?ÕF»¾æí?ÈHÎ'7Hä?ê¹tzr¯A?§Áýƒ&z8?†´ElpÁ‰?{‰bµû­?îé¾[V#?§Eq"iÁ?ënÔÖÓÙ(? A¿ßVý?œFPü"»à?‡¼çÙ@ï!?½wÅÓ¼Å? ‡QºÕúAGN4FGL J0500.6-4911¿ÖÑøì̃ÀBý@=ݱ!À:­Ž!–R½À<Ÿù¬ÿ§ë@ [»=XP#?ürùà0W?À5AU_ØÙ?¨äEdc+ô?ì¨OÌû@Ø×¾˜V£¿ïEFáeá?ïÒÖ0ù¿àFÀ¾Ìƒý¿Õ0ÀRŽ¿Ý"¡}=ÃZ¿ã•[$AGNbllPMN J0500-4912?ï÷Ñ\Bdî??›J5&Ï?#%€äKœä?rO'ð5?Kñ.¦Bf?<–¼ff¡?ïåޙR÷Ê?k6#šeNÀ?3	ö_>¥?@uۈ5K?gÀC¶êá€?hgøÅu«Ù?ﺃl(?ožT@€m?P2,1ü«ä?7r¿ ùd!?~±¾¿È÷8?nù 꽗à?ï̍Á¦?Sªqê'Kr?Elbíµ?*%ärÄÌ?wë#W¦Ž?R¿î¾ÌEt?ïîãѲJý?R̀©å}?7•™bL+?(ßí^¤?\RöïNK?Qw)ÈGwN?海Ð9ñ?…9¡¾)'Œ?Di,$Õ|^?Z0…^¿?"Wù0˜ý$?ƒ8ƒâg~?ï"û÷vˆa?uBű'eW?U™ЩþÒ?Jb©"$F?ˆMހ	—Ý?sæ_¦öÒÄ?ïŒmA"Î?n"BÿeÈ?U+D͘?B]›í5š?ŠB*2]¿1?mK¤±Þ\AGN4FGL J0501.0+2424¿ãâÏ—àÌÀ%Š|àü.ºÀ:à{ö£ðÀ<_c>"¹†@!W¯K‡'Ü?üÄ<"¸?̒üÇf[?Îìì¥@°ý¤?÷éä4È^©¿ïÿôA…ÜM¿ïï&"è±?ïÿü9¡â=¿Égâ<u§¿âð!愯¿Öv"œ;AGNbcu1RXS J050107.1+242318?뤇ÒOv=?§:ï³_?^ÇJ0–ñ?Xœ'ï|ö?Á0R fÛ_?›–"+›?ëT"ŒFõ³?¾á‰ ¿W?€CPŽ×?‡õ«Ã[›?Á«D?4H?¾Qq?ëê²´ÙÍ"?«±üöaûÛ?}¢ýn4?}Îj3âôï?¾Ð:ˆš¡_?«n6ovÝ?é°õdVÒÜ?¢5™k«²'?ˆ9:¹ód?v©¶™Åéx?Ǹ–Ì'›?¡ãUõ–J?ꥼÝ7ö^?ÁÍÂÜðº?jûóe`?gó½ªÚ"|?Äý¾Û%3?Á´¬ÃJ –?æH–ó³&Å?ÏÍÅPä?%Xmï
©?š(fÅi¨§?҅§U*:!?ίÖ^˜?é;ÚÂY?²Úà߆ìK?‡AAí÷ž?'ÉJÀÒEm?ÊFÿ|ç $?²_ϘV&?â–T \?³ö‹ƒž‰?—å³ ôÚB?"êwòCÓ?ÙTü
?´'˜ï$»vAGN4FGL J0501.2-0158?íÂ"kÀ9J]ž@ÈGÀ7­†!ÐýÀ;íZQ@x…v!@$Q2øzÑ?–Ö+Ú¤Q?¶"À%@ϼ¡Ÿ@‹F¿Å¿Êɹà<¿âl•õ *­¿å©Æؗk¿åFC¡+¿êңܺî¿ïÿ½ÅGóAGNfsrq3FGL J0501.2-0157S3 0458-02?ï¾\²¤?uYIÿDǚ?^5E´x˜Ç?c±/Ô?yDU"Žò<?n²Ÿ¶¯?ïÉ]žŽ}?~°<Kg®?MÍÂΎí?aå®
P?wvÞܬW?|0x–[Jû?ï´^Yv?ƒ=Ÿe½÷U?p3øóvÑ?{}
ºgž6?uíœÐ®¢K?xÏV]o?ïõùž^qÈ?=.d^?5ÐfíSøY?%ÿ€<]›?M1Röѵ
?5ùÌ~<1?ï¨Cc,%?ç‹2"R?^¼Y‡l?]¬
á`§½?'œ/Ê=¾?{'R¢Þ•Ž?ïˆÄ"÷
?"Ì–1ŠZš?^žA"9Í
?ržåRÙU?‰û/QJw'?"ªº,[B?ï˜uˆ÷5?‡ج?yn²&a ?'Kšñ—˜?z¯Ñ‹mÇÝ?|{Xpñc?ïéà(À(?VG£j™J?G¼ŒI-un??%ÌA³eà?`0´¸4ã'?QÕ5¹+AGN4FGL J0501.7+3048¿îŽóðÜÀ@eށ*7À:hÚà‹ÆrÀ<¼²£UÛ@!aB|§E@	ý¯Ã¨?¾!°¿Pˆ¿¤¬Ž¾Ê*±?äõé@ Ú?ý÷þyX1?¸Öf~'%?ïËKøüր¿çKlD̸«¿ái%}½ðç¿ÛÀ-Ëë%¿ÌæFÆbûMAGNbcu3FGL J0501.8+3046GB6 J0501+3048?í
Î@?¦~"_¼áÅ?rj²Å÷Zê?cm³‰E=Á?¶ ëü˔ª?¥ÂVûˆy?奮/+<?Ãfüóc ?wS|?ÿç
6:¢?ÔXNX¿y?ÃYÈåàó?í}À½ŸÞ,?š(¢jÆM?x!˜j]O?kT°¾É´?²àgêÇ?™‰a™÷-6?댶‰`Þ´?›pc8‹A$?'‰¨ŠÎ$¼?vfëoö6?¿7á"kBª?›ÂkewÕ¯?èeÊ£ìs?¶¯oÉÛc?…à…ç5-ß?uªT|*M?Ì``vüûX?¶)=©€WÙ?Ù_γ=ð?ÆO@1?àb?€"¸
nÖ?‡	·V?ãÅÍæ9?ÆP¶;eÜ©?éЉ­"K¢?ªK%ȀQ?†T5cz~?u<ªŽµ5?ÇX˜% ?©Î«öȱ¦?ä±Øƒu|?¯?ø)Òa?¥1œIì?"ž¡•
.?Óöoó?°§ïL…gÿMIXED4FGL J0502.4+0609?æóöªÊLÀ4Ü
Ð=š•À9ÌTæ³^À;¼Ñy÷Ü@:꘺¡|@jŸ±
Ï?¿Ô‡×$i—?•[ÂéZ]?ÒØöî‡@çzÊÒ!¿Ø¿o˜¿ä˜±<MŽ(¿é"ø!å-¿åG†§NŽ¿î"6©	y&?Þh!Q‰`AGNfsrq3FGL J0502.5+0612PKS 0459+060?ïî"Ææ¯?[Ãã2T'?4³ o}?(ž4š»˜?]­Zëÿ?ZyBÁŸè?ïçTß­^?h#ãp~m?1Å#Yšø?=a"mqí!?fr}Øì=r?eáóìö‰Ç?ïfn,)\?‡¯•g,uY?jE-$%?lïM²
Ïd?Ó)¶œYž?†®Ylžw?ïÏÕIŒÕ«?W™Î`·?>>9•Pî€?$ÀAšý;?v1wŸ[hô?V_¿©â?ïÞ-ˆW§?ià d@?E…<;'?<ºF؅ò?lq5£ëJ?g—îEÞÍ?ïºqýåÒ?'±ÉÇwãè?CãŽT?Uq'ª>?€%€WÕ/A?ž?ïãì׌Í?9 Q'?vYtªtÒ?x™9'\6?—-;@€ :?Œ<Ü[3x?ïj‡ÐÄS,?y-ôg5?Z	›¤=Ã?K;¿¹ònÊ?'l,㈲?wj›5mM AGN4FGL J0502.5+1340?Ü^qš¢IÀ0»)^ž	À:&=²èöÀ<0B½ê²@)û'êV@rÜ£Úe<?Á͒švä8?­Ê­¸µh­?뢱Èd@¶5?|푿²çgWÒú¹¿åœ|m8è¿ÝïU"qD¿ã%‡
¥Úð¿â<
½s=¿él¯áY¡²AGNbllPKS 0459+135?ïçh µƒ?V_COgž®?:bd¼&¾.?+'üeˆ¿?eK"–8—?T:3†­í-?ïâ×àÙ?jƒ€J	°Ð?4%«,ë*™??‰È¢I"É?j£jŠƒÃA?h|£rH?ï¤ý…lU?w+
jöÀ?]/Êu?e9͚ìÄ©?ƒÔU0Þ?t?÷Wó?ïw¿¸êë?bƒ	f.}Ú?T´'8x?1Pö)?Œï'¦?aý:)õƒ?ïË,4w'?h|Ýíwº?Oýžbž;
?@Ï|oãÜ?vj1Ú)à?eé¾:±Ùa?什?!d:?"~*<…?I4ö.Aã'?[Éù"ÁF¾?"}`Ðe¸µ?ƒŽÊû¿¾?ïPtô7Ž¦?…Vœö™šˆ?h4÷Ùaí?fù"(TÆ?'êŽ×à?ƒ$¹w¡ö?îà*«,ó?O(%õÈC?h«3ÿvñ?PVð‰RÔ?¥gL4Høf?~¤î=^%AGN4FGL J0502.5+3438?ì<䗙º&Àe©>ê!À8ïíO#SÂÀ;m·‹(U@¼"ŽðsE@‡z³$…?±1é\$™?À9×|©ñ@_;©#z@(ÿZ¾'w¿ÃžvãŒ+ó¿Þgö^k›/¿ãºÔ¢Y0É¿äÅÃù¿t¿é"´À;™ß¿ïù\wÐ6AGNbcu3FGL J0502.7+3438MG2 J050234+3436?îø¿šgÓW?"ÿ'	ü¦?i%Iè5ÆÒ?c½¬$^ú¤?ÃcnC½`?"É'Uù>—?î—ã÷ê:z?¦£Ð½èÆb?QN€2¹˜?aº1LzÃE?¥÷L€ Ê?¦?ëaê)?ï$C£Ą?ëKƒ…1ã?uÚWOù6À?züNƒ'd?–õÉEXÐ?Š	XÒ;"?îîï-cª8?vÛbzÀ-â?suX:·]?Rÿó_LJ‡?DÄJà2Œ?t¤æágI?ìU†¢Ï?²ü
€9e?'·(BÇë?'TÝhÀW?¸¾nÁèý?±ÍŠÇJ«?ëvùðW§˜?ÀӋ¶_«•?i9mKÀBZ?ZEYp°?Á¿2‰®Ù·?À©{¦‹çÍ?­o©?—¹˜±tÿ?ƒÕ†›ž*?†Z
»Ú\?¡?!¼¶?"ªQN†‰?íh"Ð×ò?'êšÏ4í.?ˆ6/UÇÌw?n£™LºY?±µD"f?™e5F°TAGN4FGL J0502.9+6533?çG=:j@,¢ÿm3	BÀ;B§½HËKÀ<¿]K4²@"<}ðÿ1?ú4ÉÖxG9?Îý"û|ã€?µG@†Wó\?íà8Ÿƒ¾f?ã£éõZ=A¿ïê¤N(ÿ¿ì-ã}"S¯?ïý©®º"¿à>qTÖò¿Ô;‰"%¿©æ"'ØäAGNbll3FGL J0503.5+65381E 0458.1+6530?ïr)Q\©?—¯žT??FÛuª®t?<@ëóÚeÃ?'=ºrB—É?—˜8bk?ì–ÖmƓ?»eýϒê?‡ƒ:•NǓ?'‰ùÊy
ó?¸_!ùçòt?¹øAôÛÎa?îQ¤Ûʟ)?˜|ᑥ»?v襶xÇ?€ y}\7?¨EÎX?–À¨\ï—?ë8!>5'+?¡à‡eu¶Í?†ñ"½`ë?yŽ}bR™Ï?Á°i>ÝáG?¡aŠÍb™´?îz&AJ?¦MZ¡˜2ë?Oûæý¼ý?S÷Ä*
†?¦¨njc"?¦§¤¸öE?çÁÀŸö]?˜…¼íܒ?žûÏX<?¬Ñ†'MAt?Íš%'?Ês™á	'?íœþ0¥˜?¢†Õ¹ÞÈ?{®+¢Ÿ?‰?€Ÿá€?¶(5RmK?¡ý7[ˆ}B?å.-…§ÒË?µkÈ:_Û?Ž§fA'"?Šwo"9?Ô®lÒÁ?µœ47®Ü¼AGN4FGL J0503.1-6045?ïø¼âÃÀBG¼Â"çÀ:Ó^†žSÀ<4¾ÓåÅÂ@^Æ1Ó@.v]Tní?ÓÁ1ùwOÃ?ÙE~ð ç@`Ũ]_@†lQ÷?ïûŸíp±¿éq'Šˆ"ž¿èîwÂYV^¿è(¶½–Îä¿æsûŸóû»¿ïÿ.ÿqå¡AGNfsrqPKS 0503-608?︯‡J?G?†yÉP³¥?vÂæ:Ð?,?ƒ	ün€/H?iʬ_¼¢Œ?kGl¤»°?îÈU&֌?£!}>ŸA?Šð.ªè?–#£Â>2Ô?™}DiЕ?–ÓŽV™·?íEP¼°õ×?¢ÈÝa©?¡õàO2?™¸¨€ü»?ªäC[Ö]?šª \iRù?íít°8_?ŽÆ–²Œ?"£ù¤.8œ?wPŒ-.?§V¸+Q¨Ä?Œv»xZ'?ï^€"e?• ©Ð•Ñ…?'ÈCZ†?"ù0Mµ?vp´Qb"'?vµí*ñáP?ìF­õØ?¹HTBýu?¤ª1@ž5?°qICÛy?³t×8"À¦?­?"–ãÚ?ëÁ¥scò?§'¯½	šº?¥3
-ü?šúx/%W^?·^\<ýór?¢EÛã]`?è&—"LA?­/ЋÊÙ@?³=ëu%é@?Í¥v£?ÅÆ«ôB»?®S3eªv-AGN4FGL J0503.5-1116¿ë½Ô6xÀ=âÅ\–À:˜Ä0FéÀ<id»k{y@ žMQü?ýHò'hûl?Ď:?ìÕ?¬
rIÉw®?æSò@#Ü~@'Ä{D™ã¿Ý'NÜÜåI¿ÜK(\ëhn¿ßÁí@	ÛK¿Ñ·üƏ›ê¿â=U–4ŠK¿Ôf%ƒ-ùAGNbll1RXS J050335.6-111504?ïԙÊÁÚ«?kåQ'ŒÂ?8k6Ðc?2Ò,z+?t,gG#z?iF'v—Ü_?}1 *å?vƒάÔ?KÈKX¥"?Rt¶,l°†?}¸^Û×?s½lÉã&–?ïˆtϒ¿?p·U³ºÿ?^:{c'
l?`"Î…XtÙ?Š¨Ñ:²¾?j¾Ü¦j­?ï-|Í¼?p¤P9ø?Y~–½ôÓ?:C.§£5?˜¸Œ£çÑ5?ps^‡õŽ?ï³hőD6?wˆë"©
?I&y9¥7?B´¨›ßò@?"<B:Š?uã³õä"Ö?ï/öé½½?—Ço çY«?]×¢÷bãÕ?måÙî[Xd?˜#¨'
"&?•œy´&+Æ?ï	¸Ì é?…äNä4`?k2'ìR?pg$j?švÆVP?ƒt€I­CS?í°-ãE½­?ŠËÚÃâ@È?nRŸ£Ž?WэP1?±ŒÍÜ÷z?ŠÞ/;PëAGN4FGL J0503.6+4518?g"Nô2V@ŸÁßeVÀ9¯Üöæ{ÊÀ;Üè,¤£¹@ ¹uj:[q?þ•i‰0–?¿â=ž4?»ïÒ Ì=Ü?ý2Ú}wØ@%™¼Úç¿ì¾²Ã6K?ÛS®=j™§¿ßväOö7¿Ú"¨~cÞ!¿âX>à»l'¿âì&ďçAGNbcu3FGL J0503.4+4522GB6 J0503+4517?îÖb»i«ž?Å,¯r£?_CcïI¬?L§OEÄ
?¡Ÿ¹-£'?o£™î?ë°`|äÏ?¾9Ñ%)¸¿?riۜŽ—?z½Iœ‹!k?Ã]mµ?½yrGE8ï?î,eZ'ŠÆ?"v	+(Ëò?}³Iüy+?rº–Üìþ?©ƒA(ot?'tGr&%?í,é0H?…"×HæH«?Œ!¨¤×îÇ?d‹e·ßfÃ?³úc¡Ï˜æ?"ß‹DL$?í<wÔð)@?¡Sž2Ûu?w¬Ÿ‡Ñ?fYh±¯6ý?´ª¶(©? ±õû­%Œ?䏹"?Å~žX<¤m?†tI$¢{ß?'±~¸xÊ?Ö.VD…@?Å>s¶¹™?ëÙ3Ø?¦w‹'½)?-[Y²?Þ"ƒÛÆS?Áæð`6Þ?¤jP3|·¿?éEø/¯£¥?›Vfu:2?ž¤Ž°«…µ?2{[úªf?ǍluÛ5?›,l÷MuAGN4FGL J0505.3+0459?è˜óò´­À4Ü9ÿÖ•À7jD†AÎÀ;öÍ0 @ØF·õOM@'Ï] Å?•€RY#?»\•­%è@#VŽÅ*A@ÕhÀÞ­¿Ë*(][Œ¿àèû6l£—¿äüÒï%½)¿åÂψh﮿ëQþ'A·¿ïÿ±[W>«AGNfsrq3FGL J0505.3+0459PKS 0502+049?ïzxŸÛc?Š/Lbóµ?q4ށœ¢?w®¾º%ƒZ?ˆØ`r¿6Í?'«Ü·XuÓ?ïËÈu­R?wãÅA} ?M*÷ã"K?_ݔs?vv"¾ƒšg?~£ÚZ"ú?î'%Q"h@?¡Óýw–c?£'²µ½?žš•p~¾?•Pf<"…?"¸Ög/ƒ?ïÏúrç?eähháY?Pš|ø¶ûù?ESbº¹z?sÜ'2ÉÖÎ?bvŠsŠ1?ïʆ:[	?'èMWe†?ƒZxÓÁ…?âX­q¹ë?•yrð}û?Š9?*§c?ïd´§Å	?¡è‹Í±¬¾?t­it««?žnFڅ?Œ|EiÏN?"ó%i*—×?íž-Hý8¿?¤µ½31ç?©ãÄ%­e^?¡&¶b¨Þ?˜rΑŽd?—¬JF+O½?ï|íÐÂ>˜?;¼ßcç'?f2PôD?^]ú——¸?‹7÷…`'5?°µÐþAGN4FGL J0505.6+0415?Åðu™½´À50ɧ~^«À9Ì1p»SÿÀ<KŒÆL€@ ËE05ÒË?þÇë¼|?¼¦ÂÞ¼Š?¬.Eã?ï왡&UÕ@.	™Üµx?ïÒá锄¿áݳÍêÚ¿ä…™1"οÚ{$
¦\¿Ú;¼ïŠ¿âsÂóáAGNbll3FGL J0505.5+0416MG1 J050533+0415?@î?|ŸÆé
Ö?Pɔì[<x?>öÅTbÅ?‹½UØÆø?{g"†%‹7?_qª'?€šAeÍ#?Z¶¹5¦`?`qÎ÷õg?"qT­¶š?|ÝrŽt@Ô?îá¬úτ?‹´ö£R-‰?uÅx|^çi?q}Òb;Ë?žY›Ræ´?‰òÇ)Â?íK;ܾÌ?‰{¶ª''D?'áT!?bZÕ žÕ?³cDñ<;ò?ˆºÕD
ͨ?ïõâ+?‹èQÆBÛL?f°ê·¥
?U$êEi?šÇƒë:(Î?Š'û×Ù«?ï	<Oø¡ù?—Sõ
Sw?kÚhžx?p÷è"@³?›]2ÿêX?•Án6ùÃ#?íhîö¶8?¡"¤9/Ä?'í?…'UÌ?{õ½+!r?²Zà\Þ? @ë'á+?é
¦N]Ûþ?¡êAÿ^,w?–K+ŠRþ?€Gp·5&w?ÉUs,¦?¢UüHÖהAGN4FGL J0505.6-1558¿ëg'ЛbÀ>n¾‰¬½À:"À';¯À<~iœ{Ì)@_ob¹]¯@MWoÈ?¿Ê™@Ù9?›¸œÇªÎ?ß¡'à'§b@šP¦`§`?ï'ɨU@¿áÉåX4¿ÜÉ þé7¿äæã>SLÙ¿Ô'üŸ"p¿äÂßäÆAGNbll3FGL J0505.5-1558TXS 0503-160?ïÝ7È2"+?b¾‡û7Ÿy?;»CÆÏ?+ê9P\Œ?oPϓ` z?aæ_Xg›?ïʨ/è¼?r]­]°Z1?BÃ74.Yø?ISžá¦?xSaÝ`?pL$­ö©-?ï˜èLb·¹?vna¸Náö?UâòÁ¼˜?P2ô»ÈÕ?‡°†ê>?u^'àu™?ï²F{m?]{*ŽaÃ?B°@7È*;?' ­>?'NêOeØ?]2¯Í\?ï¢A¨Û ?|¼$‡î|B?Tš¥V¿ëð?H>;؟\?"ÜAYȐ€?{pœ¿†?ï[
yøáË?"ÕEÛñÐ?NµgƒÊÑ??eæ¨>űÿ?"©…@•H?"f›íL?ï3ÌmÏ?‡:™YùÕ?bÿùhïÕ?b.K†RøE?—M†hð&?†¯¹ø*?ï
åöj?|¿^rL´?Y
	È¿˜¥?G'6ߧb?œ²p©V@?|Sç;ωAGN4FGL J0505.6+6405¿â$^óÅ#@+kJfUŸoÀ:Í*ÀêÀ< {ÃW@+î¼@žß(Ã?¸¤³~:ž?Ň>£(ä@`ì>'Ï@	m8?ï³ÅP˜¿Éü.dAs¿çôß:šˆ¿â[?î¿êŽ›~¡¿ézNW‹ØAGNbcuTXS 0500+640?ïÅX™õ	,?mÒ8xjÀ€?c¢P'¯Ï?Y-èÙcW??s‹aâæò?f¥Kô6û?ïÛdùš,?sOé dT`?C9®Tdƒ?OK^|aˆ?ơ¸yvî?p'nóh@?ï[지"?ˆC¹Që'%?{mý™©Jñ?€º¸\W5È?‹M×L£3Ü?€"LÓ¼®Þ?ïÜÛ×<ùl?P¯ÓbØ-N?HSSºiTL?0Ö×	D¾…?mSÕ+?N''x³?ïœF䄾/?|'ìnº00?rgÀÛ1Qw?ma˜Ñ§@?tÌú|ÚÝ?tÐ)Ù,T?ï"ÄiÀ§¿?Ž*•©ÎÔ?U¡Uê‹?g£ˆe&»Ð?ˆZ¡Ù6Æ?Œ2ô¥Ø?îÕb´™éå?"Bïí!ü¶?‰~LO?†q¹üqU?˜ÒêH2ɬ?‹u܊‹Ýå?ï=×Àµ?rD£1è~?e–xAx!ý?S¦Ý£sa?‡JëýÝ=?p²P\ªIAGN4FGL J0505.8+3322¿Õ)õžõp|ÀGlãËÀ:f÷ù¡A.À<­-@ l"
qË?þÄØý\·'?ÈÝ5:I|÷?Èϐa³'?ýÛs©EH@â²_¤¿ïÿ	*K-%?ïþY¢2ÅO¿£Gt!©·¹¿æ^ú+ª¨¶¿Ò"Üޒȿíñcºº{'AGNbcu2MASX J05054288+3321355?éµJç¦9?½;¾ÿ…?'Óî$Æhò?~{4*áIk?Çý˜Øº§í?¼AKÏ·8?èÌñs—Ÿ?À©Šä`?iXcE>_?pÿÐÚtgr?Ìj0~ì?À€D
=h
?ìgÙ×]…¨?¡èåHxýˆ?†¤¿MÄj9?{'¿dÁäÿ?¹ì™WÂ|?¡,SJÔ?í¨±d'z?	œêd•ß?€*UEv?e‡UÕåœG?µÝjU%¤¿?‹ã¸¨{ÕQ?ãHÞ)°Ak?ÀáH¢ä¤?"]ríusQ?‰:{&Á?Ø(l~6u?À¶—ZF•?àÖ1S(?ÇIf¦R9´?ržåÉ
?'I[(ȳ§?Þ	"<"¯l?Ç1Ø+ì~?ç!€õé§?°=£Oîf?š¹•às?‹qÃâyy—?Ðff³µœ?®å6gO'e?éV
¥9NÅ?¢¸k'&›±?Œ9™K7ƒF?|šî3öæÊ?Èä;ÖgL¸?¢RS½ò]AGN4FGL J0505.8-0419¿ïÁ‰ºJárÀ9f?x»Ó€À9·iþ¡[/À<œüûhÂ@«uÄ'aÄ@Ä#°ß0?µcl6	&?›m=ù"\ò?ä\õ8ü Ð@…ìiJF?ïïNlta¿Ö"vÅTÉ¿ç9.ŠWw¿â¿üò¿ì)ÞJ΅?µmôÐ!AGNfsrq3FGL J0505.3-0422S3 0503-04?ïÓË­y0ª?pÈý1³õ?AŠÛ½+?3@Òþ)œ?sèÍÉøã%?n»'Säâ?ïéÿ•¡èH?iôuzƒéT?2'£¾3²?D'£m}¬?c®5ñs1:?f*Ѫ¢‡?ïV˜†&Ó²?Šókå?w×'?Ò@p²Áp?ŽÐR^ÙI?†¢&tÍ¡"?ïßH·JÉ?M,·2êýð?BˆK¤Í"B?&¯'æ;:Ž?lԐ)8?Jîh
zâ/?祖i?€ÄÖF¸•?RzêsÓ¿?D¶ٜ°?ƒLˆl:¸?€ôŸÃäû?ïµÚÉJóU?ˆ‰6?A|Sp¿ ?Râ}g­v?qŒR'?‡WŒ÷¡l?ïÝT{ϧ?'?4aÔ?{=oîµ:?€N-Š$Ð%?˜Ôùq9‹ä?:|ä¾AU?ï¦êÁ:¯?l/Q…?[‰,O{0?F3½÷r,?ƒßÉ> ò?iN|/9AGN4FGL J0505.8-3817¿ïVmC—ÀB/@Ý?á—À:²'f™'À<ª; †ô@øáі¶?ÿ©òâáH?ÂâÍ)¾ë8?­#Ú¥¨p¢?ë)õœÏ®ÿ@	n»·¦Ÿç?ï¸Â‰|ëä¿ä"§Ös¿ä#ÁÛØ‹¿Ðð~BP1œ¿å¨Ñ F1¿ä3Û._"AGNbll1RXS J050559.9-382059?ïöîAo>°?BNv]ˆ@?#/8[@,¶?oŒÀ;³?O{,w†>é?@¹ÉÿœÆ?ïל_$[]?pBǼï?9uëÖ. ©?CÑ vÃY?ršq³/Ÿ?lù¶¶"Ä?琉÷IÎ?e‡'pS>\?P¨
¨·[?SÒæŠï¢Ý?z'6—ûL?b¯Yô6ùß?ïÈ&º©ß?U%åa?Huâ`"•e?*§ZÅØ}F?xÝæZ©x?Tj
ŒØ4o?ïð'ü"†ž?RÑȟjÃ?3ðXE_™?%ôüˆ)¤?Zϋ6^¾?Q	j¼l?z•X¨?†@µ¼_Î?E®¥ÿ'&z?T0¡}0?=7ì7?…[ÞY.rï?fž?tA¤ø3ä!?YÑÛka«?X®¹i(D»?†ÀÞ'S?r€wc€¯E?ï^Ƀ0?tg©a½|?`/gÕ.ù›?H–DNñá³?' âœÄ{­?sȘp¿{AGN4FGL J0506.0+6113¿½¹ñ0ŒîC@(1\FRÀ9®ð©Jç…À<&¼ßï¿@@ ,µ?½Z@'.B2ªw?±"Ï?úT?Å^ïN­?àPž¨ø@Rïl_¿è'ýº*‰?¹SŠk©F`¿æ–!W=ª¿Ödéc±UM¿æ}º«bú¿ÁSæ.Ã7AGNbll3FGL J0505.9+6114RX J0505.9+6113?ïγ€0Î?h7åzeÈA?Ehr?@5øNòL?uèiՖ}æ?f‰t-}m?ï½ÃGÆpÆ?ƒþdéöh§?Q}pýnÚ?]â•ñ,?|Ö¼ÓÆM?'§W}Vv?ñìÁà?}>NÍ?bõŸe˵Å?hÄÞ
¶OÉ?‰¡[¶³P'?x'ü1?nO?ïnN¨7IÌ?l0—3´¨?pw»ÒÄR"?PŸðuÉZÒ?Œ0wøý/Ö?i]¦)ò?ï}ë™R.?…`…æYG?YÁÛÓ3û?P÷µŸ–f?LÞE"5Œ?ƒç$É,i?ïI-öÞ?œ'~ä¦L?b¶L8'õ^?râCõTØ®?"…UmYo"?šŽY"M`?ïáÚûä'?Žeå7&ݺ?n¹çŽåK¢?qð'"á×Ê?šŒ‡ª‡<E?‹¥ÐÑ"Š?îy˜œ2j?ˆ›­áÅÉ?‡òØsJÚ­?p7Ææ¯Ê?¢q°UŸ»?"çOGK½AGN4FGL J0506.0-0357c¿ïgёhÙÄÀ9-DŽO¹À;{È0…ÙÉÀ<â¾|§ñK@  czΨD?þñìVuX?ÖÐ^ÚÖÑ?éµ°P•CÊ@
h¾/?ÿ-å^0´¿à­Îod;ê?ï"E¥%¾Ö?Í91d|'¿ßCµA?æJ¿ãð"aùð¿ïÿvä܎AGNbcu3FGL J0506.3-0357NVSS J050605-0401520?îÄ 
èÌ?šÎÚë‰Ö?…'çͨç?w[ºé…ø?œØ	?–-\¦â?ëÚt† Ô³?¸Ãhµ%?±-ØŒ~"?±ˆÔÎ+¥(?¯ý|F¶?¨œJ®6û
?ípð_›hs? 'À;Ùp?¡]˜ÿ™<?—4~—­.?§ëœq•b‹?–àƒÄãM?èTýÐнr?¥›Åµ)¸£?¾LäEu'8? 'ÚꐺÊ?¿-/¹<?JšF×n«?íäÆxAQ¦?¥åoª	?—·©Yh¹?µ–FË7ï?¥×ÃÍ@? ÌH¾@à?åè»ä%ô?Éj…£ºÒ?Æ )Beøz?žÓÃiª?Â<êKã®;?ºN×ûfŒ?ëУÃ,ÿ¬?¨®¡Göª:?ª}±¾ué^? äo1ºWí?´<	]
ï?£?Ñ^ÿU?àuÊEo1!?µÊ7xëÓ?ËHùƒ3?³Ñ~•	ы?Ñoî³Z¤?²"aÓ ý:AGN4FGL J0506.7-0857¿ÁÑ$øT\pÀ;O¯§"YÀ:3+y*ŽÀ<Y^¾Ò@"¾ì‡@Ÿ.cÀ™¹?¸3°ÜJÿƒûW2'?̦WB1(@/DŒ?ïÁ6á¾vs¿âØŸUd¿ây,Áÿê1¿å3+;-C¿ÞÚhH¿â¿ÚÖ­@•qlAGNbll2FGL J0506.5-09011WGA J0506.6-0857?ï܅þöÚV?]<ü9ëÁ×?A°¨:,‡Ú?1ÕO^à¤?o
Ö¾!h!?[I™öK³?ï×o¢)—?mÂòûUx?<¦Ð4?D‹¢ÙL?r†äµ¯Q?jÉèaí̝?‡L"?u'¤¾tõ?XQåÍÀ«?Aþ×Ó0¢V?†‰a|Â^?tÙÎûÁ¥ÿ?ï¶ê$¡u?Y
[¯¿{?OÆÕ¤äÄS?0ô5%k?€I	nÇ?Wò!F~ðó?ï¯Xz6õ,?sYÀ8ûÁ?Vë"]¤†Â?Eå-¸d?LnÜï<3?r6³$?ïƒô I$?†^Þ÷`ù?LsÚc‡Bk?YËs¢4Uò?;ºTõÜ®?"íÝç‹?ï9ƒg[·i?†•"hO?g
buK¨?eãy÷¼´W?•îF¿ãøf?ƒøkÌ,]?ï2Üíðø•?v3ºÛžLã?e¹­†¢1?O¿J7`†?–í,—!j?uˆ[ŬԫAGN4FGL J0506.9+0323¿ç9mþqpÂÀ5\ÓZ…‡"À:wO"¼
À<ZÀ2Š–Ç@ Ja·Õï¶?þÓۙï)ï?ÁÏo¹Ì?¤)JQ1öÈ?ãO]¶>–@Û̈́ؗ[¿è—¢KïÃ?ïé%=QD@¿ÛÈ*;<ìð¿âP7…¨K
¿ãJ™aj?Œ5¿28!AGNbll3FGL J0506.9+0321NVSS J050650+032401?ïÝîÅñ?['ëœ#T?Boš§ŒÊÂ?0´­mQ*?nG*ýªÉ@?Y¼ Œv?ïÈDý?v؟¹MN÷?Jwñ×vIþ?PiÞúy•?x­ö†!GC?tŒ­Œ8‡¯?ï"S÷uš?t[ڎ"Ò2?`¤Æç73¬?\×èòåÀ°?ŠÁÐx¨¿?r2O8¬?îùó7*õ³?v%I9´?rF>5—Qñ?RüZIC¶#?œ0	«?t÷²¿0ˆ-?ﺉ¢U«?p3­;?V€×'°ñÂ?HÄÐ#žó?}^DéŽ,?m_Á¤Ú#?ï`k!ƒÉ?£M–n"?^vyBöY?i²¢B¢If?'46tx{?Ž
œD˜?ïQk¿0?ƒTˆaÈ¥Ö?i÷œ]@?`®Ñ3˵?™vÜKß?j¡6®J?í'y`­Ù†?Ðt±‰££?'êG‡­ É?jÔ ŸÐôÞ?±Žìi[2?m?á{âMAGN4FGL J0506.9-5435?¹å ²`×ÀBb‰üm¤HÀ9·zn['nÀ<D€bï@ }ëišù@?öb¼'«A?¸p°íOF?ÁÃÆé³ãG@ýöÀ¼R@èWº§¿ê°Öâz^¿Ó³(¶ØnÁ¿É1£:৿ÇLíCÌ¼¿ÕH[¬¿Õ<{ÜDdAGNbll3FGL J0506.9-54351ES 0505-546?Ÿ
CW?Š€K Ú"?fFI"ŒR(?n>¾±
†?…"…ÊՇÏ?…'ñr¯±?ïÈIV¤ì"?z+Ã~˜h?EŸ"Þ"?PH"Ù?c?y'r>Ç ?wcü<Ȧ?î‹$è(;?™…Ë÷ÞË?qT¤"Þ²?s‹X?¥#è'£?˜§ÁJn«]?îXÏ©Ø?†Û`Õ¥2?_«Û}ü?D%è7sç?©zi8äß#?†gó,¨—ž?ïpՈ»®?œ5ÌV	•ä?€,IçÚ	@?†s\—Äû?–ÛÀSÄW›?"œçV¿?ï/!
'©`?–—˜!DT`?d<Aò/?~'ÄŽÓª?—"\çä4°?''!9â|?í¾ÕÞ÷Ð9? $ã
è?>?[¿?ƒ\hø›>?¯ÃO=û?ž1o
ÔÔÙ?ìÐ¬;˜ï?Ÿ±OKuQï?i㸎^Íu?[o¾½7x?ºÂ\Ørâ?Ÿ€ÿwwŽ`AGN4FGL J0507.4-3346¿ß#0Ÿb¹çÀA¦
á'6À:˜CÖ¥éÀ<'">iƒ@ ÈôíÓ,¸?ü¸<ÿ?½
uyÔ­A?å›G;]?ÓwE|Y@ãòóýé$¿îY»È˜Š¦?Ñ*²Æ'Ii¿ÚˆüéJ1¿Þf*]㋿ÐGòká%¿Õ¯?ˆ¬ŒAGNbcu1RXS J050727.6-334628?ïÔQkáB?eú
2?=¨JÇrâè?-ÿÄ+ðÂ@?süÅyû{W?dúc·ù?ïÓbÈC†?q³VØù†·??Jadè×;?LyUø|?tYõº5×7?o<vs'׊?ïqЯÛOr?{¨È+jv?aóaœâ(F?löâö1?ûªâ•'?wNÔ¼ä
?ï‹ÿ*u¨?dßµÌeÇ?I9­mîúì?0Ï*'س?‹lš{úså?da¼;ç®?ï©Êi˜Â?vö™²=´?QSZ8Í?BÄ	"èìV?ƒcSüwÑ?tƃtK¦Ñ?ïpªT\¯?ŽÝ©þfƒà?Lê!6º?Xà¬M/n'?'
62îŸ?´Œ
Ñ'?îô Š}áœ?‰Ü½wó–5?c"mvv7?`C'³
?Ÿ	(B"?‰cÊûro?îÏI|á?'×™"ôÜ?]S"µc)?M¸H:Šm_?¢ Ï0éÒ£?'¿^>¤AGN4FGL J0507.7-6104?îúǺqÞóÀAû‰?¯BxÀ9Ry§‹Ê¤À<¡V&}B@Ä*m @ö‡{‰ä?°ÅÜ~ײ•?²=Âno@@}ü…!=@ü!3Vn¢¿âMQâ É¿âò#žjº¿ç¤Ç+£¿åíuÿ‹í¿è˜b—¤ÌÔ¿ïÿÅ}M2¹AGNfsrq3FGL J0507.1-6102PMN J0507-6104?ïÛò<¦'?¬( ¦0ßO?2bÑOAj©?9û˜]Õ^!?pà´}Ñ3?¬*9€ÓoÁ?ïÝçnä6?p¿˜†u»?@p͕‰å?K€Ó°}X?mü]ËŸE?l¾0Qm)?ï•W'ãòÙ?ƒzNkñX?[©s/èE?^®Ûï+PÏ?‡H&#DŸ?'æ?òºÇ?ï×ûªÊˆ?Tu=¥8w?Umé%<·V?:yZnœ+Ö?n<õqSÑ?Qõrì²I'?ïÅ<2v ?ªñܒòÉQ?[¤þp>œ•?ˆOçè¿Ä?vx´Û3(â?¤àZ뉥?ï—ÙÖÔI?†'º;Ëi=?RÐÜF?bœŒ@RD?‡¯nÆpâø?"þ
ÖLò?ï7K]mæ°?=Ò¨ÁÆ-?eÓIÀ÷­$?eè+A(Å?–\+"a?'±"nŒ?ƒÖ—Z?u£ÌѾôÔ?qX§x¥é?\´°9+åH?"ëP¶õÌ«?rc2³ë,DAGN4FGL J0507.9+4647¿å•Ykߪ©@vÊa¸¼À:	ÅDBO0À;I%Ü3@ú¦‡é˜à@á~4¹E?ÑÚØÞÓàg?ØÑÐAÌS*@准qž©@_Êe"Yi?£Pª"¹ús¿ã¹%¨05¿ä`‰þ#r¿éÿ}Ž¡¿ï÷x§±ŠQ¿ì)	ä…P6AGNbcuTXS 0503+466?Óõ-¶Îx?Àè»b8¦²?œÀÕqá6?œYxŸýK?åb…Ó‹z?ÁIJ¡¹Î˜?á]ÐT¹H?Á[¹œâî?¯–+"?¤÷ï
µv?ÙQuµþn?ÀvI™A?á«ï®½Üß?³ú>sMíƒ?´?LGá~?Ÿ®÷RFÊ?פÏVÑ?²õð-`F£?Þ#ŠêæN?¯'ؾ	i?¦K*ó4×?º7?ß·Xu?°ˆâ'n¾?¿>wÆhø?¯^Ì|
‹¡?¢÷µ‰³IM?¡S€Ð7?êèµ®x"ü?²Ñ`…PâF?ÑMY®¶Ðü?Äعjy?¼-{t|?¹j®ß î?ãرc~™R?Å!'`9?҆GËNP#?°ˆç"/j?¾èÒU¼ŽÖ?¥ânÈÖ?âßÁÏ¡F?³Ž~_£Ëï?ÌÔ¾âî-?«~Ñm²?ªî±£ ?'iXŽ'?çå-Ž%?°vˆ9ÎBMIXED4FGL J0507.9+6737?è*M±í+@/ÉèPðÀ8vÖFÉ-À;›òâáH@!Š¿¨X¤?øž¥Ýtº½?ŸL¬^ ÒÑ? qÇÿ™¹á@ÔæŸê%@áY¡±ì?ïy¼NÐG¬?']$É8¿ÚþÜÇÔ¿Ë`À	Dø-¿Ð'¦ÂÌÊWƒ_—±AGNbll3FGL J0508.0+67361ES 0502+675?ïqü£uO?°+½êæü?N(¥$«Œ?mqa'÷V?Ï+Hnˆé?®¥³fýb?ï՝|ŽW,?sݐSÉ¥?I?£ôÕ?R'…;/®?r	M=kây?pâ6•
7??íã©óƒð»?¡ãX'â˜È?kI©Ô´s?z,¸±GÅ?°cN ?¡*›Í
M?ïBH@"?t'gœü?fÖÝÒ§€?L¶²nˆI?"Ü¡(•\?sxV—H'?ï%º¶c˜›?¤™ÇƒòÏ?X¨–Ô?b«ÿê4?™¾)'?£±ß'ÿE½?ïˆYôÏ0?Œ:"²Ã?^UcJÜSõ?kâß°—ž€?ŠÖd8)`?‰@ÿ·vG‡?íTI/Žì?£\Ñ2ÕBÒ?n¾lŠ¶]?z㿾o?´gÃÃð¢m?£»´œ`f?îg…qˆG?Žy¿±Æy?x¤(´GG?g™&û¶?¦z'µ£?ZŸ&AGN4FGL J0508.2-1937?ëŠï®µÀ?2×@ÄnÀ;*í"1{À<µrþ$]­@xC¬':×@åPäôá¿?Êú8À»Çl?ØHC{)ìã@C"¡@µÚ,†Æ®¿ïÝ7~ŽÒ?ïÔ£"`š¿àé.AÜÄ<¿åºðáÿäÒ¿íøwÀ«×4¿ïÿý±q&´AGNfsrq3FGL J0508.2-1936PMN J0508-1936?ïV¦½™~?ƒõ›]-?w¸µ–ê^?páô»w¨?ŽyõÈCc?~]Z'Ši?ï
A^;–ü?˜ÿ»È©¸²?A¤5??†Ú#fP[?•˜3m3ÂÍ?'fMP9?íñ¿àÖ'?œIÅmsP#?™,
²Ñòþ?'¨-‡2ö?¤Mü™5t?"¸L ¢æ?î¡Dðí4ï?~Üò®Ž–W?"³Hݸ" ?uû¦û)?˜$1B?rÔde'8?îœ36Iy?–dd©XñŒ?‹yïމ^?ƒô€‹yÈ?žþ\œ "-?'Á¡ø;?ìó<Gp5?´\'úÖ&f?œªà1ç*\?¦"É"¹·s?±;gɸ§C?«‹¼ð¸n¯?ìf_«[ÿ?¤2'|ޅ®?¤íð'\‹?—pøÜ7]k?²V
]šóˆ?Ÿ&I…ˆ?ì×àÜÏ#i?—c0&
…Ð?¤óoàÎçx?Œ'PâÖ?­Ž'Qbúõ?Ž‹q«AGN4FGL J0508.2+5211?íû €~@5#ŸAyGÀ:ÀÞ­ŸàÛÀ<4p¿…¼m@ 
z?â@I´˜c9?Ō[ØîÄ?¨ÉÀ°3å?äù]ÿºŠÖ@mà0ù¥?é"ó1»cï?ïøø²<(¿Õð¡¾+IZ¿æ
gAؒ~¿ç®±Ž'å"?·ôƐó'ÄAGNbcuNVSS J050809+521256?îb9¯èÕ0?œ·€øG€Æ?\v>¸Yó›?K	F(àc?¨ø³Fj?œsòs?ì< ‡t~?¶e0ô¹?l£{HW?ƒžid	¯?½5ßí³C±?µy´ôÂHà?î+q.°0y?"Ûš†X¾?x0Õ†6Ž?sÉ8u–ÊÒ?ªBÒs»õ ?"^PEÒB?ïљ[?y<ÇÑ!Z˜?uR—_j?["ý`AJ?˜ÉKQ¸?w9y	Šz
?ì"ü>ÝéÞ?¬	œ|q?sʨ²G¯§?mDÝ¢Ù2?º#s€2óÑ?«žƒ#»ñ?ç"ñ¨G?ÆáÁæý?~ËK9"œ
?¶"˜l?Ñ@¢ï¦
?Æq"Pô(?ëNo³'pn?¥Qn]…á?†´ò߇ÄÃ?zä.¦y+†?ÁZò!û?¤DChøv?í}í"Ti?•/¾Ÿè‡ ?ˆÒËAñâ½?yë/Kº™?°ö:Œ÷Re?"–?Ê%pAGN4FGL J0509.1+1943?â¨)ƒ Í¯À'ý¼#1]pÀ:	ã<zڒÀ;Ÿæ·Yž@E	¬§@†'QúŸ?Ο¹ï$'?¸F7qÜ;U?èì&>ƒ@ícíbt¿êÁ¢Âi¿ÝXl¾U¼¿ècya•Ç'¿èêŒeÔp/¿ïû'Á^Á?ÐC	Ÿ»òŠAGNbcuTXS 0506+196?ìkÞþÜ?»¯)xÊA,?eÁª0÷ãâ?b˜†2Î?ºæ"·N?»X0vHj?îéšYCNp?¤04–®¯`?iÁ.†¯€?wW¯¢?Ÿ"°?£(·—!v?é"|äØg?¬§÷Èà?š0Ö?Ž…Š ³\l?Æl	«ïl?ª…rýðӊ?î3[eñ?ˆ:Öè
a?q¥ŸŲ?V›¾ÙY(?¤øm"ïÎ?†óÂïy+,?ë<ìïÏR°?½ªÕE1‡?i•ÒWUÈN?b±¬Éà(?Â¥ôõú‡_?½vÌvKòÙ?ì҆hˁ¯?½Øs§  $?2§ø y?Ž‡sì-?·Ew¹x?¼¬ÎEƒÿ?ä~YqáCÒ?´hL`$Ë?¨&~•\?"H
¤ ?Óþ}Jې?³tðÚ؅?ìH5ø¤/ä?£'aXZk#?""ýÀši?t`ŒT.!ô?»+°ƒ§%/?¢¡pW%ãAGN4FGL J0509.2+5550¿ïÎ"þæ-@"Ÿhß½jYÀ:.¶ÁȍÀ<~'­N@;2'D"@˜<ÿ?ÅùԂM͓?¿í½‡?ù7ýÒÿõ@<!í%?ÞþáEª¯¿×*&ʺϿå$u*Nˆ#¿ÜÞ硺Or¿ç¶?A´U¿ïþ±`à•'AGNbcuGB6 J0509+5546?ëId"÷jÒ?®ùü¢%Ïà?~…¶Ü>T?q§qŒŸâ?Áæ?ô{D?®näÐ~Ñû?ê2£ÉÑÎ?¸ìÎn|NI?‡Â¦Õ­¡,?‡ ¤ÔúÝp?ÄYų?·í\i\?ìünis? sÙoBñ?ˆˆ¼ÞŠgâ?}4ˆãˆå?µG¡)Zí?ž"×ûë?ìÏÛt|Ëû?†7ʚä	?''J"–‹?gÈDÕ*•?µ9?É#?"I'žüñ?åQòo.ó?»³ýYB͖?˜ÆPSKú?'¯^ÿt&ß?ÓÛî½&Un?»	p0•ö?ãÝ)k*½»?ÈEbW/‰?™•c‰O:?ŸÛňìÀa?Ö¬Vð§h?Ç}Gã]KÏ?çð0÷f ?°ÚD‹š?£^Ø%ôÆ?•sÜ+ö?Î̹…áð?®¥ÙÃÖ.?çýW¸3ôµ?›S´û"_K?¤l]g¸k¯?'w"Y?Êï‰ÃÁ>?š4ÃûÄÛAGN4FGL J0509.3-2917?áu…tï	À@ïßã*dÀ;	üȽÀ<»ÃlѺr@ùeä@|ÍT¤?ǼƒDÃ~¿n$M$;—²?¬fóªNN?þ‰ð¯*%¿ì–ŸV¿ÑΗÝ×·¿æ
|?ì¿Þ;	ÛØ¿à8èê9Å¿ïó/lÕqAGNbcuNVSS J050927-291339?ïÏ~;€oã?s/ÓN¾vj?>íõ‡¯Œ?8ÅO"D?vRÉ	|?r8F
ò"?ïÇ6'Ñ=?vãÓ,@'?F q'`œ2?RfÁm,°?y ¨Ì{dî?så>qùl;?ïnf	Ê.7?wôûj#h?c¥ƒ›ú¸?Y­p	Ž?}œ
b?vkEn*G?ïÄÝü¹¾A?VÝmJÝ|#?Q—¹g«?58Œ…\,?y+<âèü±?Ua×ÃÆGÞ?ï ]LP)}?{5E.߂?KHÃÿ¢D?@úž—@ó¨?†4+þ!Ö?zöüÂÒ?ïEZÈMŒ%?"þ¼Ì›?\r«&µ{?sŒ3,
ˏ?•"_Ï»˜?'¹¼¹T+?ïŽË›†?"ê*ÎL©?nné¸X,?f8­ ''?š1P¨?ƒ7;h$nW?ïaÌ(7+»?uåßÔϘ4?eäݔb$?S¬°Ôqý`?'	ú5ØØ]?tZâ¦>UAGN4FGL J0509.4+1012¿îì"ÑÍMâÀ1>°ÙQ?ŽÀ9YµÂÅÀ;î:Ç|*ô@s·ìj÷Æ@×~¶ß%?³<ƒd?¹1¨C«{n@:$¾ü*@Š_[^?ïû‹[é4â¿àAR—M¿ædÊðSº'¿æ†Å~ð¡¿ç'uÞ©¿çBž
A¢bAGNfsrq3FGL J0509.3+1012PKS 0506+101?ïð'PÛöÈ?PÇuˆäÞÆ?$Ý{t¤g­?5:ôØÖ©?\A®Ž,ÚÓ?O×ñ(/8?ï彊N.?nÂß(¾ý?8—ϨpÀ?DÔ2,ŽåO?g/|2–+V?k‰U»à¡¯?&ÂGÊ?xkàu¹| ?dÈï×@© ?gĄä2?"mzSƍ+?t^'`ÀÓ?ﱁ¸?`!ªäÆ?Y[®5ÍÂ?:7l«¿0Á?€tF	4î0?]£ä¬Ø‡¶?ïà×2xņ?bY—–¯æ?6
b8ÑÄ?)Ïï6]"T?lg!AW/?a r¶áÀ?ïÃ:ðÊ`"?€íJ1ƒ±?MpD¸´«?[ÄÞ_%
X?z´"•?}€–+n¬?ïG¼<[Ðá?…³ޔÏ?v¶²»Êã?vÿїi?'ZËÅ¿&?€šSU£Æ?ï#Ѩ¡Ü?|÷c%&ž?rà ¤ÞÂ?ZξË•'?–Í¢Ê?µÀ?z2όÏïˆAGN4FGL J0509.4+0542?êP1Š€fÀ3¡zÌNøŒÀ7K(û¡ÌnÀ:î
N@êÙð¡¾+?ÿîȺïT·?–~1xï?ªŸþ…+£@H×°´h@'í~<Q¿Á@WH'>V¿Û R›X`"¿âÚ>û=y¿ß,J
æ
¿å#ªß½s¿áͽ¸‡ÆAGNbll3FGL J0509.4+0541TXS 0506+056?ïàïUQ¯å?c‹Œ6–×S?:>áÉÃÐ5?1ПA²¨?kÈΩÞm¯?b×
±;y6?ïéZ?ͱŠ?i"ñȾx?3`-'T©ú?Aêz\§?d9º¯ëtë?gÈF¾rò\?îIÏ7ÇRÌ? ùFf6'Ø?|EæÏçcC?…Œ–ä£ý"?§ÚOª'Õ^? L%Ö»?ïíEexw?JGüZ
?Y#þÛÇ'?
Óv+âr?aיµðP®?IÑ·
îÀó?ï«çq`6ï?|Ÿ×IF%Ä?F<þ¡"&ç?Aeíl»?ƒ¢SÎõv-?{g«Þ\@š?ï¶Y›|Ȩ?œ<tþË?dáCpÿÜÄ?›-Užy ?zb{]Mt?€‡/›6oX?îu 1—+?Ÿëñù¾?xÃKë *?"*yqôû?¥"l}"?èJ4_5Î?ïÛÿÊûçB?bsìi‰(?*C2…¿lD?#¿Ir_üé?q.ÑY¡ù?bx\áAGN4FGL J0509.6+8425¿îA‰Å¨ã@8ŸB»früÀ:ö,ÂãÀ<‹2§òø±@Ö ‰ÍÉ¢@`ù$C¬'?Å^I·Y¿³árÌ%]?ìá¼]"Ùç@ËîX^¼?ïúwàŒGL¿ç³ï†¿é¯Pð³[â¿ãƁŽàØó¿ð?ðAGNbllS5 0454+84?ï݅,áE¼?m@[ójÜ?dçƞœ?eÑI»JB?[¹×&jìi?cbAhS?ïdˑ?¥¡‰åâì?'NÙÊÁ	?'ߟlª=Ð?–"¦"óªl?Ÿ[zZ!?îÖpÔBQ?–6™øç£?dcƒºÇ?áJ ? Î½''?¢b_"p?ï¬õn¬†?g¾.‰‹E¢?jpÛ¢ºý?Uàh<TÇ?|LÚÙàM?aÙÈÍ}"?ïÄBæAŠ?d_ä3Ì+?võ«‰é©?}W'•=‹É?[£‡•žTð?Z_­¹.ö?íÏPJθé?²LÝÛR ?'x[ú?¢F©Éóª?ª†ôæì÷?«"ü‹)´ò?í̈8$À?œÎ–Kgyº?'[sÀÌ?Œñ–~µ?ª	Âñ]¤?—œü{SB?î•i1$˜Ä?'0u8G§?Ž`!±^9û?èö>?ž"Èûޒ…?Ši_é?aNAGN4FGL J0509.6-0402¿î!kNqlÀ8k™¡ýjÀ:'Ò¬áÀ<ZÆã~¿ù@ &|'²wa@h_dêed?Áb¥üÿD™¿'=<Ÿ/?ÒïœePç¤@"‡®‹?ï÷z>Š¿ã8Õ3£›¿çdú Å‡ß¿Ö—-ƒ›Ö`¿ßÖ­3ªQ¿Þ³Ë>WS¤AGNbll3FGL J0509.7-04001H 0506-039?:JÍj?nH—ÇP?MÍ'Ø?>·c+Ñô?}ù8£Óò?kû½Êu?ï´S
áQá?y" »?RYÅú»¿?X=Ïø0è?€›R|%?v½O{}Î?ïh­¢~ßH?xgïêgt$?bÌ\N•M?aPIc2>À?À4Á†P?vē »WÌ?ï»Ãe?s!µ}iþò?bOá¤&8Å?B£ô¬.ہ?šž‹\DBˆ?rä eª ?ïnX©©?ƒC'£˜Ø?`%JÛÒ€?Q©ÙùH:]?0Azïkz?':#+Bâ?ï6f/£ r?">oLJ"¼?[MRm/?cÕTã¬?—{E>Ð)¶?'ÂBã²õê?î°Nˆ½íü?ŽØ—Jï?oöôɂß?e²òØ8‰‰?¢û¨%¥5l?Œì,\¬Ã?í'7ù…VZ?'©ÈΫî2?zŽ¼"‡ø³?e!¯³Òvû?µTq€Ò¢?'à(¸.AGN4FGL J0509.9-6417¿â"ÄoÀA˜>}QÀ:N°÷"0|À<"ê"]ðv@ Eúأŗ?þ-Aª?µ¾ S¿ƒ'ëÆ&d?Ð`¼ÃÀ3·@	Ý
$¿á¨†Ò¸©¿ã·S½v¿à*®"Óa<¿Ù‹z‡…šß¿ÚoUã·J¿ÜM8'}sHAGNbcu3FGL J0509.7-6418RBS 0625?ïõŠ±§àã?aîBÃï?"äBN=?40Úl‹W+?RŽÄê?^懜ã™L?ïãl.§]?jÌÀÛxqa?1XËÚVXO?<IÂÔ¬?jÅz8¤c?hZù«g`?}¶}€?p¸ÓÊ°¦p?QÄ}ii{?c5êr¥?|À›ˆÖ˜?l)¦øhæ*?ïӚB¥°Ã?R6±~z÷È?63øúg A?—#xá¿ê?tϟ*ù6?QöOДVà?ïìMX¼?WÇ}[¹!ê?4a´ïû²?&Q«/Z"?an'"õņ?U÷…*Gas?ï¡ÏÆQ]–?"†Ï÷Öd?;D‡²|ª?Gc6ýLÊ·?†±ê$IÖü?ƒê"'tZ?ïTeKÍù?wL‰eéB?T%(ÄrrÓ?V˜•Ÿý0?‰fAš­z?vC¨Fë¬Î?ïƒS%ä7š?q¹EƒZN"?NóÈW5mE?<ºËFš¦?;ùóyô^?qw>xâCAGN4FGL J0510.0+1800¿êÈÛ?pÀ)p—AЅÀ7÷uôxãAÀ;F­)¬@žp•@­@ÅÂíP?žs_Yhj?·«#Ú¥¨q@]¢r†/@xkv›"?¡ˆeûÖ~¿às-õÐú¿âKL.¬»µ¿â']ÂS¿æâZh+b"¿ê½4D«+AGNfsrq3FGL J0510.0+1802PKS 0507+17?ïè‰lXvl?Y¨á5'"°?9^|ßGŠ?0©l@ —?dJÏáÇB?W…oz3ê?ïè‰ø¬?r˜ùOÿ?2È%ÓO"t?GðÆ.,^?eúfãäÁ?q>ÞíH³Ç?ï²âë>ŸD?€™z®¥U?e:{LŒ«Œ?uõ׿»?{ñL¤lˆ?yáN—ó;H?ïî1jŸõÃ?G:c7Çã? P²"˜?ÖðCa|?`é"ÒÃQ?FC²ò…þ?ïÕ@ä:V?kÌ«'´?;yÉÁáù³?2ÌSOš??s§ñutˆ?jeZÉ4qä?ïÂ)yå¸ñ?n†_C÷?TG®6'
?{U¹ÔMMÔ?yåq†9â?
OÚËÍz?ï—tïÒFš?‡–ì>wÌû?q	0†Ão?}\˜Cí"?žCýÑÁš?mìB
?ïÕøTºíQ?cC–»Â[(?0d¿5»ŒA?#¢°´åA?sý‰Ê˜æÓ?bÀQ†0äUAGN4FGL J0510.4-1809?å­>kÀ>05z5PDÀ:¢ÏîÀ<œÀ<uªŠ'¥a@%ònZ@5ÚBU?DZ¼»‡«?ÀêB> ?ôE;ÞÓ_Ž@
åð¦p‹¿àsco;!>¿×!˜ r¼5¿èà<K	鎿çŸÌäu¿ãC‡^ƒ˜ü¿ïÿšÏúAGNbcuCRATES J051015.50-181227.8?ïì¿Èéz?óÞ&*P?Qqp±Ÿ?Žz6~¡"?VƒóP?JW WÓ@y?ïà	àmW?k
@,4K??5Šì$?@9̅ꪐ?mA$é;"å?hƒYV''ã?器-áî%?uB¹*»?Z/?c8MÀ?_'C]?'ŒšÅw?r¥ê0S?ïÞ4<·Z9?Ii®ùÐCô?AŒÉ½X¯Y?$b¶ðà?mh±—Rõ?GîIZªU?ïÚ¦L¸óÛ?iq!z€ÿ	?A#`Ü/K?7[ˆÏrÒ?pˆm¡ìíà?h+b>AŽÖ?ï‰Ç"Ž?Ž>s!B—k?MÙvU~+?[AÈh4Tð?‹°§"<Ö?Œ?ð/þJs?ïm8ӎ»x?縚í€?c—Êށ?c¨=?Ë؟ؑÁ?~Ù9¾yå*?ï£Ì˜Ÿs£?gÇ먎a?UùƒhB(?B>½†–•¾?"M©jÂ͍?e¶îqhÊ-AGN4FGL J0511.4-6804¿åX…à19ÀA%×ý'w>À:Ï&رÝÀ<.šLGp@p¦d]þ@ºV€?U€?ÅãæÄŗN¿mÜ^y?¡'G=VM@'º¹Në ?ð¿èZ,fWѿ듦¹Ù«¿ß|"¦Ò¿ÒŒ\š4Ê¿ïø×aütAGNbcuPMN J0511-6806?ïo‡¾¿‡¯?™yÄõºm)?>nœµÎ?8R´àl"?'"'lÖLe?™R×¿h7?ï±Ñb¢{Y?‰ Ó{å®?LM+¶d^r?R~ž(‰?ÆÔ¡h¬"?ˆíëR	gQ?íÞïT"µb? à£ðêÌ-?mKÈ%T?¡?wábçD?°'Ò6? ÓÞʋE?PàÍ?g6°™üó?7!.ŒÑþD?!ê1šSi9?‰bw¤î?gìË#Ž'?îªÕxäà?¬˜ä!"?T"ŠËè?Qo9j ,‹?¤®"+V£?«ÆFšÊðI?ïS¢˜µ‡Ñ?å,Ãl Ç?UŒ	¡:?c:šGv܊?"2ìI;s¤?*Äý,?ì»qÏ6oº?¥fDB$<Ë?vΥȄœ:?~7à…È?¸·‡'g}1?¤±ÏÂڜ?îž\pˆ*?†½šæÜԓ?T°ç ݆‰?GJtPBø?¥t±¾å"«?†Â9,
ÓgAGN4FGL J0512.8+4041¿ïÿúfþ†?íJf@%ßãÀ9N™û¿(ŸÀ;Å(wŽ'@0—²Ž³@TZDïô?µØJÀ~Æì?©ÚˆÍ¢
?ñËÏÇSH@Ñá»Fg˜?É"üÚ0¹¿ç¡Ìþ¿á¹	ÁŸÈ¿åF]É^ٿ༰À&Ì¿ìaU_Ø؟AGNbcu3FGL J0512.9+4038B3 0509+406?ïf×Ñsáµ?‡Ýò@`?P ?#ªø?EͳóXúº?'ûü1¶©?‡9_Js?í–9Þ{©w?À~9x¾úô?V':J[EY?o×Ð(Oi?²ô("I[2?À&Þ)
?îˆ|S–2º?•ÌÀ¸ln?€§ž®Æg?…V?*Kÿ?£NSZêú?'ë*݃'5?ÃéÙ?d$•¦÷?Q`‰R-°!?2m6ÓëhÞ?ˆf}ßëÐ?c."ã`…Ñ?îmä°ªh…?¤¢\¢øzì?dÎ}ˆ¸<?bŒ%'^°p?§ÔÍ Pr?£ý0HÆc?êv¥zg>?Æø"QšÂ?aî"uƒê?}?¥šð?ÅݯÆà,Y?Æî`)z;Ÿ?íÐä/P5ß?›Ù)$Ý5?UŒW^Ý?'»×'Ý?®œ|#ÇBe?™¶Ö¢UÙ:?îÚ7¿'…1?"ÄŸèI?h¢he5š?Qê]clò? Ò]}±?ƒ—hgùˆŸAGN4FGL J0513.9-3746¿ï¼ÜôQÀA[¾<Q‡À:ûÏ[óEÝÀ<~>TÏe.@)aIñæ@>"DÎf*?ÕzOÇã?ÞóÞ>d>Ä?ü4E]c@3ÝKue?îñïÁ™gð¿ÂtlùÓk"¿å6Aü$¿ïÿî—ø¯ª?ïþ{¿ïÿ7Mt'AGNbllNVSS J051404-374607?ïÁïiú‹?yÀr^?`ÞAX.?hnŠ|ÕC?vÈ\Žïò?rŠ†¢0o?ïPù#º;È?œŽo…N'
?s†9R"j?ƒ¥/[®™?ÿ;7x7*?"âÿJ?¢?íµ þI¾Ý?Û°{™š?™½KñN/?"‡%¡ðÃ1?§ÏJ L¶?–OH°vý?ï¸ñ"x[m?p¼ß¹?2Ó_Ñø?2ø}‰¹?2ðK6Ê?p\'5·e?ï;	¨@N?"ÒÍik-¿?yc$Y?z½Ì¡?'Fü<¡Ó?'» Ë)C!?î '""Æh?µøihyf?…•ÅÒò%®?š~&ŒáÄ8?¨'eR÷?²;Ûà¿\?ìV‡—þ'Ò?¤ÌLe²'?¡øõ¢úƒ?˜iÃU9IK?´OµÃ…v-? zÓ~lŸ?îÍê'6áÐ?™5—ê)ð?Uw¦mÓ?`-ú.BÕ0?¢x™ÌrÉq?˜°QŒ¾ÌAGN4FGL J0514.5+6247¿èŠOXûN@+š™0¾
íÀ:£>ºOò‡À<uÌÿøsD@µø/°@"EœÂC?ÂnʸöV3?»ñ'Ž»F?ú|ÌQ#ß@€ýêQ¿æj8î^
?ìšÏú¿äW­Ñ_Å¿ÜXGŸ{ÛÄ¿â^zd¿ãœg¿¬Ó³AGNbcuGB6 J0514+6244?﹅ì­Vª?¬";Ù~"?o>ßfêß?¬¯Ù :Š¥?s™ôc£?dûÓÕ^¨?ïÆÄ©¬{?}Ӆ»¥¹â?M¹m3‡{?W"6õ¨Â»?xæ}€éßT?z²Yæô"Ø?ïŸæmefÀ?xŒÝ?«ýw?ašgðã++?pÏjQ{Ÿh?ƒŸÊªm…I?q.Àۂ?ïa·þäU?hú+*'RI?q¦¾ãž?Pã@Z!ÚQ?Ž¾½߁Ö?htù†Ô?ïÔþ/×o?~A¶ìd
?U˞Žrâ\?IX}¢+P?…ÑL'½§ø?}2Í±ÄÌ?ïWcm|t	?"H«Þl?a£|^@õ?m…V†iz?'ß"ÑzÉ?'¾0d½=?ïH,%ð!?ˆL¤ÕT3H?g	0äù8?n H'""ƒ?"YBfê?†ÏÊd/?î7ÈhäðÛ?…´þÓCÚ+?ˆð†âÉ?p+`%æŒ?¦€}Md‹?…/U+v=ƒAGN4FGL J0515.5-0125¿ÆÔQ˔À5â]B¡À:š¶ŽœæUÀ<^@îݘÍ@s–ñ?ùüÜÊpÑú?ÔKa}H€!?Ô.á_+Â?þl˜å>³š@‹ö~•?ïû¢}˜Ý¿è¯L¾õsµ¿á§?¿³‰°¿ÒÇÜ£¦¿åŽé<o¿æÞÛB0|AGNbcu3FGL J0515.5-0123NVSS J051536-012427?ï|]÷,è?½úÎE#r?Uí±ï‡Ôú?L[û¾NÈ!?Ž*Ëì¹7€?€Îð"º…?ïªá K?|6uj_Ï.?Zº¿ü©72?_£Ò)Cuj?ðG´H>W?xè‡'y?Ã0ÊV?–è"`›?+^`²3?ƒéüÇ5é?¡l¼6"¡?"O-·3¸ˆ?îf¤.‡Ä?|:BJð®?n¥&~è'ú?QÒ=àw°?§«j³o\?{éÚA±þy?îçyPÎφ?–ípƒÐX?h
k±Õ~»?a{¼Ž? "7É´®?•åÔm}?s‰²?›J8|Vk?l=Èr«Y?}Ÿùn@_?›2iÀ«/?–é1¡&š?íw@¥? a'¹}?‰ÙÿŒÓè"?‡…¼2™Üë?°IŒÎñD?œµ7Üo"ÿ?ì@\`Å?•NX`eÜ®?wW°?Ì<e?h™iXî2•?¼‡¡ù©=•?"Ùd펐AGN4FGL J0515.6-4556?íeQ"LèÀA°K	éÎÀ8Äb\ìj!À;ý'æ÷ñ@ƒ)[Cµ@%AÁÇ?§´Èbô…½?©»Ôàu(Õ@$x]ï"@ØëpR#?!HW»0¿áÜ_|gY«¿æL8½¶¯¿äR½ú¡ò¿éwomv% ¿ëQ­DqIAGNfsrq3FGL J0515.3-4557PKS 0514-459?ïØŀŸš?'Ð…5€â¶?cÂ^VCü?'h­}!ü?d3¼ír?n(&¹J?ïìj''a?dA¹fÉ"?*ör²?9û›3'Ú1?b<3ð™ñÞ?b¬íK)ïr?ï—[>'?…Ø€hž?]çHªçëN?j×Å´·¥œ?†lUaÝõÒ?…¹ãuŒ?ïýÂ}_ô?›ê¤
[?¸p…_½>öÉ?.*0FÒ??ÿgº²?ïÛÁÅÚ»?k
Ê%á!?F̒ö£"I?Pœ_ÁŒ?n‹þàm?f•p©Y)æ?ïÆVJjæ?ƒóK-ÿ+?KLùLñl?lž×D¡)?yk_6Á¯?1²8y©œ?ïsòPæ?†œåL¢$k?aªò9ÊMU?c‹¡wŠ]?ŽÑ†ë£ø?†Ìü圼?ïúŠø8'Ë?9‹ÒÕ¸²ä?jOÓ±6?¦}ÞCú>?B
ga·?7_žË{ÄãAGN4FGL J0515.8+1527?æ;‰Ö­÷À*!ÅXdEÀ8ådÍßòCÀ;¶_"ÊÕ|@ É®ŠA?ýµØy©9J?®èO_8Ê¢?´ß="u@ÇiÃèø|@
¸÷f©WR¿ç8ôõ
¿Ø¨ÆÞ \A¿Øc¾ÁF[Ú¿ÝbßÆú{¿áÚaàŨ¿×¥Â¼þx–AGNbll3FGL J0515.8+1526GB6 J0515+1527?ïø¶cea?8v¶‡€Ì?¹Úƒ£<a?{$Î]â•?Jo6–"?6™.ڋN.?ïáÒÏ´ø_?uщ'+Ì?<'t•"¡?J.wI…àR?jœá¨-y?t
Ž]¤>š?ï™ÊÏÐ	?'d;Ö%T8?][(g¿€?gKªº\"?…áç­ë®?€F™Ù»¶»?ï+öEŒ|?qý;ªY?g' §X¶?H0«ŠŒÝ
?—¸[Rkp?pà­:ôeH?ïñ
áWH?Má¯Ð@T?,²j[»óf?#k~Ú??ZS𬠾n?JÔ¢·EJ?ï¶u«[k"?†Õ~s4?Péð[¶¡Ë?_ŽÃÙ/p?€EW'¥$®?"uWf©?ïgT3D6L?‰n˜)8‰?cÀR1¥eg?o-O™^?oIá`Þ?†ÅüTøöd?î…6Ø{¤?Ž00êñŠx?y­W=ö`?bn?çà?¬Bª•Žt?Œ¯¾×¾-ÓAGN4FGL J0515.9+0537¿€–=¶pGAÀ2Iâ%úeŒÀ:÷ÒîNý"À<AÍ¡Þâ@Sõ±G‹/@'l6Kì?ÓaŽºú½¿",ß5N?ÂgBÚE0a?û»‡ëqR©¿å;66ó²¿å_"û-¿ã4íþÖ	¿àŸ=è˜Û.¿ã€´ÆEÊ¿ïê¶YFmAGNbcuTXS 0513+054?ïºçH½ÍÅ?pÑõß·S?<bgQë~—?-ØTvç@£?€c"ÉUÀ?pbŸûŒ?ï§YÇWÔ?ƒ<Зð?]Œ| p•˜?g΍ƗsŽ?'wþ'-uí?€ç`B©&Ž?ïMû}†µß?€¸ÓþQ ?hv˜"dô?gLèEa#«?"1½8ñhW?|Ò~ìßܳ?î™Oƒ@r?} ûr݄?bç6
'?Gs7è?`^?¥<"ja›ò?|";n'›(?ï\Ÿj`hm?ƒä,¦ƒb?MûrËç?A[ê¯Í°4?"|7Ǘ÷?'¡,¡¥×í?îîbõ [ž?£hã+N†?oÙÈdů?²ù¡¥Ú?ž8h]SƐ?¢Ôì%¡Z?î8Hµ"?'xzŸŠG¸?y°ë®
?vƒ£¾Ñ®?¤H»?7¢?4½C³W?ì%¶áQê?›ÑD¡\Àý?rNĒÐT|?d7£t""?½­^ÈbYç?›i}®<ÏûAGN4FGL J0516.1-7240?Ó|T…¤€dÀ@kè^9qÀ:gÝDUGÀ<2Ô\.Õ@|<uQ:Û@ü
éÿ
?Ãw©Å5Ô£?³'Þ
øø?ðG™ò"í?þ.zœ~Ph¿â5N`¶#=¿çv-NäH¿ç|U†DR?¿è@¦¹<Í¿ïÉéÍ³}¿ï	AÈ!laAGNbcuPKS 0517-726?ï¢cއñb?|–i$è÷?\ߪêIÁ?T%ÌöÆÎå?ƒÎ"__le?y"XíÏø6?ïáâjæ?"ú†Tw}?{1)ß®â?yC@~ð«?–—'ˆ|[ˆ?«-oî³#?¥Ýö?ãkísÕ?zoé>^­?x¿ÄN?¨]?™îL×Ҙ?‰÷¿ m?î;›³¾ø"?'¢Ç–[9u?^ªðØ;?qºÉ_p?¤nÃ0'Ç?~OpA¢~?î³%)bØp?—§\¬§‰	?tF%"4h#?f›¯Ç¤?¢D軋sö?–ORJ;Ã?í3¢¥˜¿?´Ë­Û‡?'l´²ok'?›ƒG[Šõ?±Ç½¨É`§?±©
ò/R–?î1ë×ÌR?™î	lí†?ˆù}MìC¡?wK,£ró?¨ÎòwÅù?–<x¹÷žb?ëôÊMî? KM^Â(?¦KсÿP?'Dq7êkÞ?»âq,p©ê?šìDÄý‹âAGN4FGL J0516.4+7350?í~"$Ï1@3Åf'|EÌÀ:~…AÀ<uV=ú6'@ I«w?ü΍+Í
d?¶{iضºè?°õØ^ÑF¯?ù-6´Çó?øòuJ×?ïÿ2z¦K¿çiÊ¿+y€¿Ï¡ªŠ,¿¿Ü=›{?¼¿Ý ¡€mΐ¿àÚÞrç~)AGNbll3FGL J0516.3+7351GB6 J0516+7350?ï°u)ÖF?í°aý	!?Dò¨ðmÔ?:²ÂGùb&?'ª8t/³?Pn›?î¬õXöÖ?©f´×ƒ?…]»$·M?†µ±};(?ŸÎ#Éd¶¯?¥ÂӁÊÂ?îµt­•¾²?–`®}œÝ?|Xp<ÿ"â?ƒË} wþÄ?¡§ÐE^?".j—:©%?íX<Ÿ˜Œ(?ŠA<
áåÅ?šˆ¶€+ʹ?wU)0ߞœ?­7ÚÃÍ£ ?…Já2†ü8?ïaXa¸N2?Šì¡m<]B?Xl†ó›	?Mψ'ÛàÊ?'N+]Ü)?ŠL}iß®?ìŸçûãw?´´Î€Í?žãO÷ãF¤?£
øaŠ?³NÌÂ( ?¯Y$*?íç®bÜ÷›?ž
¡þô»?ƒñâàOU'?""f²½?¬ˆ¡ÎEi?œ.'Þʯ?é´}ӕhÝ?¡/|]]N?¬èËB©?€"úsZ2?ÁóÕáY²à?ž
qí(AGN4FGL J0516.7-6207?Í y'W'ÀAaÅ.rÚÀ8šq
"=À;Àâf'@·ut@Ù ¡`7?¢[_LA?¨'K‰Á4@!Àoz@h²ŠMÈ?àÀgc¼gû¿ß}¡ku¿ãŽ¶aP|ð¿à˜ö«:¬¿æ䁦ާ¿åó
ƒç€­AGNbll3FGL J0516.7-6207PKS 0516-621?ïðQ8¤.?uï\ÝHU?–ÿvM-?æ}:	J¬?\÷îQ-Î?uîõUQø
?ïå_<"?i°zkáço?4I£Cbœ\?@Í-ÂÏ?hjl'rÜ]?gFHUXã?ï¼O‹m
?s öLÿ^?U§¶±c*?[í°NgC=?|nLÙ^jî?qÆ›
?ïíÇ@›Ñ'?BRípN}?0Íë.ÜgB?í-Fa?`ÎèU?AÑ$cšy?ïéZ°‹ß®?V[íÄn?)³¿g±?'±È®Î?e
°³$ÿ?Tޅ¨ì2ò?ï³g"ŸðÝ?ƒ˜	01Io?J"d%
ÉQ?`M†?}ԙ+Sü?'Jèú\k?ï—Pl\¨*?~ƒ-_ÜR?\ö±—N%&?a¶sèW´F?†ÁšÜ¾?|];ˆð6?ïÚËÚxJÙ?ZœÄU1Æ.?AÒ¶¡x·Å?0ã¡j‹–Ç?p_»õ_£4?X ;kbÅAGN4FGL J0516.8-0509?æRʊɼÀ7YfYÑ,®À:`œøÉ«À;÷À¬-@ÆÎi/œ@C¼Œã©?ÇÝCýÛ¸x?Ù)x¸.@H/yjO)@	†qÀ?ÆxÌ$ý»¿ãu"FK=ì¿ê{>º¥Ù¿îÞwëÉè¿ïÿ¤?åÉ?æ2ËŸAGNbcuPMN J0517-0520?îé›E|r(?³+ªaø?wñ;®
Kª?|ÛàËc??œÐH^;ë+?¯ÒC'¾?ï+YqجÌ?—]€"Ø^?µIaûú?ˆ«òî'Æü?'ºP$Xðt?ZԟÅ{Ì?í€ÚõžA?£²$?œ%Ťsï?'à®,Øãø?°ò‡½ì7¶?žÉüÙr4?ï
\KÁ†?Ë=±¶xÒ?{a_æwrB?`Dƒ¢?—†Ü{â»?{6Š¿õð?ï(!hŸ??§7¿±q¬µ?r`ÙE>k?~×_ج?–x:º–2j?¤:¥EÞ×G?íoXs<@V?±Ü5—pÝS?›E&CÄLŒ?¥Ç<4Ѩ?«g娢a?¥€!õ ?ëÞË¥¸êJ?§ë¹2Lj?¢ÎG`¼®G?˜Üd֏>?·¢ |?¢»•&t1K?í,HC¢?hLqR³?"êŽLá?€éeG?²bû'­?˜Á\¯˜xAGN4FGL J0517.5+0858?×)ùë¥À01w…r›(À;e DC%ïÀ<ì&qƒÐÚ@!F€ÞaÊ ?ý痾Ή?Û
úD5ë?ïÿÜ>Y×ã@ÝK 'ß@M T3^¿évá]ÓoÔ¿îí0º²îÕ?àÖýr‡?¹¸ÁÝõ-¿ê²÷¤ëá¿ï÷ÇLZK¦AGNfsrq3FGL J0517.5+0902PMN J0517+0858?íù±‹!½?¦‡γÃ?›GK)ZR˜?˜¹š4?¢ÁA¹"Óæ?žó(Wz?ì¼!R
9?ºø2/–àF?­'ÓVõGO?µíÙBï?§ڗY±?«V€_ãu?êT×kÈa>?°š´æ¶Š?ªP?—oZ?›ú­ó¨4»?À'jr±ñ?¬	P"Ôp?êxÈæä%.?ª9QPòº1?µ	ÁDLmé?¢ƒ،$?·/÷ƒ¶§?¢)·\ýi?ëv_«ó?¸úc†À¬Œ?¯g¤'Iƒ?±[•"L…‰?´›³²	¤?±9xÁŽ©q?æ~ÛWª?ÐRÜq쒡?Ȧ -Ð{a?̍Â6Ƽ?º¼äç±8?½ŸA'¬[,?çJ'´5b?¶ß¶œ½C ?°)‹3û/6?¡*‰B=Ð?ÊÀöLDsš?¶¤»éÁn?áã( Õo€?ÁÊÄd?ɽEóK´?¿qiÂÄé²?ζ‡8̃?ºI"¡ æCAGN4FGL J0517.7-1758?óâ)À<ƒ…@FA-À;SPßìdÀ<n"d¦rÆ@ÙZ.Ÿ¦@?û˜'3?ÓààHŠ?èö'¤‰·¤@
;&wºL@JE)B¿àÔMà½?½t˜j¾e¿ã«Þj®õ¿îwàmò¿³Ï?Bàû-¿ïÿÂ"NßaAGNbcuPMN J0517-1756?ïáåýd3?Ÿs(ymj—?p ‹‡é?vø|y0l&?™\û%;—?Há§A¦R?ï$Öº?›ÃøêlWÞ?~ŽÎz"=?‡àLÕrm?"Áuñ?'ªV9ÏWâ?쬒þ}|‹?£¢ðä¼Õ? ÕxC½×Ø?•×Ùk!Ô??²0«ê5/»? p8XSV©?ï5Ÿ¹³s?{€ß¯ýi?qá­ö›?bD'ESý?•ý5±xð?x#
œh7?îAœm?®
€.),K?‰8a‰?âãt
G?¨ÚYÏÀwH?ªËDOyà£?í+t
ªÜ?¹ÏY"?ž#|~M/U?°1;~̳?®7æ7ŠŽ?«íëò?ê±:²Ù[¦?ªÙ´a¨ì?§ÎŠž÷Hï?‹yÓþ?¾Žå"¼Ø?§†ÄõzÜc?í.ÇSÕÚ?ž|çI_Kh?ŽPŠ—ê?†åDçuD?²ÅÖ¦å3?šXZ܅׏AGN4FGL J0519.0+0851?äZ6¤¤1À/ß-@ªëÀ9:2áԛÎÀ; ˆp|iÞ@ûPæ¢`è@Œz¤áÌ8?¹óô®é?Éme^(ªC@h@µKü­»?Ез=¿áIéXÎG¿èÐn**¿èƇ~9ö¿íÕç]qË?¤7ÀvõAGNbcu3FGL J0519.5+0852TXS 0516+087?ë¿ÏNî`×?·2£š?°ê™ûäô?¨lÿ—+SŒ?±ášíµ-Q?«»Q€Ø?ì¬Ù~®?½	Á¤‰ä?±F¦	Ë?¶U"Ðï×?¥ì¦=ä3"?§=ûÆ?ê[»ƒŠtÊ?­rI3$Ň?¯µ%m 4–?Ÿ†"W†à?½G',@Xh?¦N'mÜ?ì@ÿV·È?"µß¤Úê?¢Ýηc?<™Tú?´ñbæ?‹.:U÷?æc"—¸ ¡?½Y^¸j?Á˜žû`ç?´Àãþã7'?ÅpÝIÞ?¹Äí«û­?è4LwŽ?ÈÒ"nŒG?Ä8îOÂ!?Æ–6nZ?µê)K̪?²ñû!r6?äPè¼?µ­c	(Œ€?Ài÷¦¦X«?¨¹ç'Z¸³?ÎTA¶·??²©î‰±e?çH¿[†J?©Ì…–a¾§?¶g©ðDoG?™—ùŽ?Ç«à	%Ô·?¦ao¢xkAGN4FGL J0519.6+2744¿×ô ý ÞÀÍW¼w¯À:œŒ" ÚÀ;ætxwàâ@  àBöIÉ?ë6™ŸxÖ«?éýáí›N?æ‰=–c"4?ü"§—‰!@ùQê™¿æT~<Fl¿êöDà"º¿ä)%}½ðç¿Ôr;†¾Ì¿á$ùê<I\¿ïþ«6z'AGNbcu3FGL J0519.3+27464C +27.15?ìû¾í'Œ?³ct?Rz?q"|u͇?l³lŸ×ž|?·כnD?²î9ŠI?è\ðsÚ ?Çêǧ§í?iVæØB÷ù?x«ÛøþÛ?Î&ä6\Á?dz‹›‡¸ú?é©L0'¯?°ES
œŠ`?¢·[<åÚ'?—6uæi´'?Ĭøqkø?­5îz""?ì
À‰ŒJ?¨,<6 ªC?B¤';7£ý?@à=+ҁ?¿l²Že¼{?¨2­(ýE?ë{Z"K&?½&l³)(?€¯1Qä?z%\†ïÂù?ÂøW¡ôÔJ?¼§–¥|?àúeŽË
?̊šÅ‹{?rBzjXd?"2 ªœ¯?ÝÂ*ŒÆws?Ì:nŽ±'¼?åˆ$lA?´XoV‡È¢?§lQ"  ?›™ý¯¨*ª?Ò,õbœ?³´¨Z%5?éƽ‰'?·!ÓÝÖI?4°o'Š?Imö¿?È݌ÔusÜ?·"õèîÏ(AGN4FGL J0519.6-4544?ï4˜H¿?#ÀAUa=1¹¶À:6Ô;VdÀ<~¡ÆŽÅ@QmPæL{@'@œ¨AÓ?·óTKâÿª¾ÜŸ'Íú?ò•ôÿý²?ÿÓqíLa¿ÞÍ–%œ¿éŠŸ䍿æwé`J¿åÌQ¢_¿å4јäh¿ÕV¢ƒÎTAGNrdg3FGL J0519.2-4542Pictor A?ï»d­Sµµ?wmðCâg?Tp;ݔÛÆ?GH©8éu?}1šcb±?vÕ¬
`?ïl)Hù™?"U‡q¬<?bð+oÇ"?`èجãþ	?‹hêáFÃ?ùûIJþ?î¹Súȟ?'/PSH?xâs½eöZ?stmÀðÇ
?¡Nqê2v:?Ì~8ä#á?YuDÙ?~|®;dœ?w{qæ¤E¹?\0yP–ù?£Ö¼/ˆ¾1?}.ŸlÊa?ï:aPZ"þ?'(h"Þ:?od5;ýƒb?d‡­(¯±?"ÇOUéÎ?üAÏý?îk'y`È?£ú¬ºÛn?y <¤Ë?…%`ØJû?¦汁@'?¢²}Ù.6?í>ў»?¢2◙¢?‰ œÜÞØ?'~©q߆…?²èž÷ÕΤ? ‹ÚÙÉÃ*?ë½å/^U?œpÍ@¼½ô?'0€ó§Ï_?~ä¸+?½"¶H&	?›$ú=œŽAGN4FGL J0521.3-1734?íû[ؐF×À;Ž~bÜn+À:dál—À<>'(ŒD@¢ÁÙ©ª@É%x_?Á¡??Ûã?ϘiƒQX¸@
Ь¥åØ7?÷\mܧ`W?í´5&Rz ¿¸º¦?Öjì¿å~SEÎ@¿å->â"Þo¿ïÈÇ.¥/¿ïýD™`AGNfsrq3FGL J0521.4-1740TXS 0519-176?ì42.ë@?°á_…@}? 	×*ý?˜$¢™?¶YæO?¬kòR©?èÛÍ=,~?Â	,w_æx?Ã[e¬W6s?»Ã®oXlB?¸RV>²	«?¬–‹>¯`?éxãè-Œ'?¬|±¾3´?µŽ«'ÑáG?¡´©Ýßo?¾ª5?ŸI©?¦‡4×Â?å‰o´‡ b?¡"Q}˜~‰?Ç"tôô‰)? rޞëÅ?·Ì8ìõP?•ñBqv?åŸYò9¢?Áf"0K?»dUêî ?±Z8µÈ;?ËÐmBp	u?¼†HæÆ™?á
ßÅ·v?ÈŒÄ MI×?Ò‹fiÛ*?Æd"5×IË?ǧj%kÖ?ºŒÇpŽÕ¾?åã'%gÿª?²c'؁¢1?À×Ok¼ÖN?©@#¡G?ǚkü}i?ª5¾Ç´0µ?ÚεJ$;t?ª…õoO»w?Ôz7\@P[?®¾ãy8Zw?зY›t2?§=ɵÒE™AGN4FGL J0521.6+0103?ï2êÿÎèíÀ3Zº8u'SÀ:ŽbwÄ\¼À<]Ú{9@ IKèá«V?ÿÉÉã
?ÀSÒ:
²?–8…‹"f?Ùât¿D£ô@$3"¸¿ï㸌íº?ïÿº*2Ùq¿åò³{Âîý¿ßEœVã;¤¿Òê"ޥȿá1ªlÞAGNbll3FGL J0521.7+0103NVSS J052140+010257?ïðZêöó+?Yh>ê3Ø?0oÀØÃ?#qA5ÕNü?[FMÓX¾C?W€Œ=eé?ïì@o0å?g´VÚ
oX?,"=x'–?:J£Þ2?b,›ªnÂ?e'iÇ,ñn?ï–NÂʄ7?}8â±"êÁ?Toºƒ
?V?c`÷ÁÛº?‡ÞWù6]?{êYÑà¹e?ïÍWÔ¨8n?U5¤%³s­?AÝ¢ÅÇL?)r¥izŒ?wa:úr8?T¯‰ªìq?ïà?m©%Ô?fÀmuø?C×uöJ‡è?:úb;!.¥?jÊ´Àиê?dmÛºû7õ?ïÄGÛ`ä?'&DžÓ²Ë?@²— 8t?Ròø]ü0?{à	;"Jð?€ÔFìœK?ï1aW;ƒÂ?ˆ'¼
‹#¢?Z?;ŸÖY?`ä°(/SÀ?˜2ÑÒ9Y?‡©9ŘÀ?ï€ÚH¾é=?q#³ «-?T[eÀœèW?Hsˆ­˜2>?>!Ðûª?põv@AGN4FGL J0521.7+2112?Æw÷cçÀ!iÓpóˆÀ6Þ¯\y}šÀ:­ò<ÈÞ+@]"ÿ‰b•?ýžøé‹Iu?'œÅ+	?§v™[ӇÉ@Çxþï^È@ȅ%ï'쿍4ö`€/¿ÙÇCáVF´¿ßûÛÙ>¿Û[$^.3š¿áø"ÁEZ'¿ÙÈý4s¥AGNbll3FGL J0521.7+2113TXS 0518+211?ïF´pp¼'?Î
4mb2?R²çp¬ƒ?M6ø$$P?–†¼f0?G.±¦þ?ï}ô}s{Ö?£0vúlÊ??Î"ŸÛ?O¡M@T¦?ŠÚ:ÓÎd?£!›¢†Ö?ë¶6WwW?¬îß?lܵ?±Æ@~Î?‡hÓć?À
>65`?«ú衼F?ïÑã½T3ß?aK~5<†D?)0'(êå|?AEÉÜV?vDœ¯Q%‡?aP.'¨ž?îX.üS?¡¬òjTØV?`I$"]—l?X=
<ß?­eêÃi?¡Vi?îË®¡†­?´;+6½ëÙ?Yè>žœ?xSI>K?¢uÓüïÆ?´‹r™¸i?ëqјR`?¬æÅ6'Ê?€Bè{â¡?"z'=Õ?Á4‹JÊT?¬)ZŸ]&?ï­wÏðBÉ?t
e2z¢?6•o"¸»g?-wòÇË}?ƒí`8¡ð?t@C€SUAGN4FGL J0521.8-3848¿Äq߉=À@®1¤½º
À9ò÷Ãñ[øÀ<Yñ›@T¹³?ˆ@"C'OH=?·1NA+™a?©v(ù!?íºôB\›â@'̳¢Y\¿]kW´>W÷¿åÔ"°Õ¿ê1"ÝIó¿ä\¢b•÷N¿ätSŸx"¿ïü¿øÓçAGNbcu3FGL J0521.9-3847PKS 0520-388?ïú–©Ð?6µkŸy¡ñ?íø1Ò¥r?s[Ô8?AǙҙ[3?4PMf{Օ?ïìMmñõü?iPô"‰\?(Jyg©?7Rõv-?b-ên}G
?gE¢ƒò?ï½ãSÿ˜?nòŽ_Ï'?T³Ò$,‰'?I¤!yAî"?{á}Ê5aÄ?mLæ$Ê!?ïøz\‰æ?/#çX8=? uŽõܕý?ñ§/	Aô?Iù*
rgœ?-d´‡t®?ïöÞToÕ?Fœh®pà›?'7g—ù?‡Ä¢ˆ3?N¸ÓÂNgI?Dìë0?D?ï¸ËQçB3?'Oôè}`?=š'-[ó?Lda`ú´?€àVå
 ?·í®KÞ?ï˜ò®nùï?wSÍV½U{?\vÇc?OÚ¦³åk¿?†4{y÷Q?u¿"˜ÞË?ïê'í…?Oý¶"·ƒ
?;/ëLÀÝé?)ˆ?k–n?b"\3?LÓ¾éâAGN4FGL J0522.9-3628¿Ò›í±É¼À@\] l‡À7Ÿmži3À;¦¾Ë'Iò@ðáºÅŽ@øÛÎÈO?"¸ý?¹Üä?³v¸îôiõ@ôAÿ~Ñ@U9˜R¿Ñèb8Yc¿â|Ê@€x¶¿ç°c	º"å¿çJ0i¿çäGbj-p¿át>KëAGNAGN3FGL J0522.9-3628PKS 0521-36?ï׳—?SÝwÕҘ?7Âô0(T2?-R¶ïðb?ZÿÑE¨6Þ?Qw¹3¸ 7?ïÎ󘓊6?vÞÅNÿn—?Fmø•\í?Q¿Ãҍ¹?u¸tlÄ¢?täÛÒÈ;"?ï"«*nF?‡nïOmK?iL0tWæÕ?v	šs4[L?"¦‰%´îª?ƒíÒÊËg]?ïùk¼Å d?1PÿeÀ?)&BBv?R€QÆH?D{oñâ?,qËÓóÚ*?ïÔ!€ê\f?nžéەƒ[?:`Ù#ãh?0"«tòÚ?tI2sì¦?mÍúæºÛp?ï_5‹Þë?žMè—ãÉÚ?a´î@†I-?xD{²¹]?'â°Ýڛ?œÚ$˧¸à?ïZ¤î%Pá?ò°ìYu‹?r¯(±Øà?€IùeŠ‡ÿ?&vw°¯™?‹¯[6?ïñÕqzÛW?M{@?;Îxfä-?4©J"®gl?Ua›îl0?GÖ:v¤wAGN4FGL J0524.5+2839¿ÍÂ+Lùœ¨À*Éòý¸þÀ9€ŽÌܽÀ;âF¼|ó@ X#8lÄ?þV>¶4ž?»àçáÑ?º ïZP?ÿ¨Ec·_}@ {KÆÓ?ì½q +Y¿â¾È'«hÏ¿ÛþcEÿڕVß	æ3¿ä;uÂ#ü_¿ØåÑëð~ƒAGNbcu3FGL J0524.4+2839NVSS J052429+283918?îcM¶Rs&?™®œ¤Õ¦ª?g¼/ŸÃ'Ü?{ó<þ,#?¨Oa£DNu?˜"œpÏÝ?æU«3t÷?Á•¸Š0×?}WïF«ª?~í˾&?Ò߂<ì֔?ÁXR9ç5?îŠ
…j
?",¢å¢? iƅôk?s©¤}›?ª£R£-?'Èk"¿œ?ëzj½
<)?ê«©gÊ?™+8ñkÆ*?o¯ºÆ{?½áÛÛ;-0?‹È»¯Õ+?ìg¥Bf¤F?¦E»påãx?}Mo–ÞÓ?ls
Íö-?ºíþòJ?¥íçX!%Ö?Û
m¥'Ÿà?śÖÍNh?†‡' ¢Ž•?Ž0¯VaŽû?â ªåá&?Ål&ö¹Û?ë\Xátz?£-Ê/çãÏ?4ÿÒb×É?ï'2þhÔ?À›OÃÝ?¢V=œ•7å?å¥û'ñ? –%öӔ9?ªÛ½Oˆ&Ë?‡"ÈuPïD?ÑX'R3¶? ŠÈЧMIXED4FGL J0524.6-2819?à›þNáÑÀ>c…@FA-À;"ƒ°jÀ<Ÿ˜!ÊU#@ˆâÖyt@®ˆ#Oa?ÛmN·ó÷´?̳ɛ"ñi?ðPêÄ.™@
'S6³ÆA?íJa¸¼-¿è3hb?_¿à5B!b¦=¿ë•›¨g'¶¿ïüËÝäw8?ïÈm54?AGNbcuPMN J0524-2818?ïê‰ZB
?jùCMœ?NdÛAQ?dë7áåV?[»mŒôèC?`]þ\j¥Â?ï½!£é©§?~'VÕLiº?S±šÐ¦û?^Iéj«²-?|'Ç]ॄ?ys¤Š‰ì?︲I??­"ù é?x2É!ºÄ?|à·¡%®Ø?–pq?"ú?×¼×ñŸé?ïëÇJ.?F££±*ŠR?'d—%Ñß?ó'Q=Ւ?bÂlSì¸d?Es¡°Aà ?ïÔKQ•§z?p†!N"²?K;·žžj?IjOÿ
á;?rràa«?o2"ÔrX?ïM­OƒöÅ?˜	Òü6¨Ñ?aRŽ›ûOí?v²m­"ìd?" @ý,X?•7X'r'?î½Ì£K
?"ÞÍLÆÏ?{þAiw×ï?€®ÌÒó)È? £mœª^þ?'ÃZiJIå?ïÁ
Kˆj?i€AÃi®?2'CfÎ	?+æpÅäs?~\	BUY^?hÁ¸Ãgµ§AGN4FGL J0525.4-4600?éjT.wÙùÀ@Öb=ú	À:bøwu'cÀ<dà?p@Ðÿ£ä¡*@'÷
èöÏ?Ãþuf^ƒÄ?©‰¼VÝÝ?ႣžU@#?ÿ·.Lïqè¿á÷ÀBû¨¿è¯•ÿÜſ㲁œøŸ¿à¡?«;®¿êp$ sRˆ¿åÛÍátϋAGNfsrq3FGL J0525.3-4558PKS 0524-460?ïg{ÂC1?…45˜'|'?b¥$÷5?Rð{žIF?»ão›?ƒô[´ö?ï™Cã&!õ?ØÄ#ºˆ?\k‰û¾À+?`·z‹"'?†!•õ÷È·?~§E-£}¦?ïLPëÕу?"°?¦È§?rr®Ûƒ?tƒ_²šA?'ðFI´³?~²àÈnLœ?ïIkÎ|œ«?o¿}Å,äG?s‰6Ì¥ ?Sðj¢¿iÙ?'ð8'jn?kÒ'Wm\G?î'Å¥§?˜îŽÔɺV?y€Ñ¹ÿì?l"œÕ»?P?£³š§¯³—?—-ëi¨·°?î¼PÁl$?gxlõ¸?qö·?{¦'0@p¦?¡üöê-?›H¾§ôdç?} E?' œGgÖP?~)=ďD4?z^ۋŒ%?¡²pÜÿ"?ç Ô7—?î$ü£g?‹"¦Öè?‰G£˜?s8·[ÀRè?§^OKÚ®i?ˆU/ÆççxAGN4FGL J0525.6-2008¿í¸ÌjÒ1À;ŒŸ±À:Ý
s†	šÀ<§Ç'#©R@ÚRý¨â¸?þÎE"I$?Î`ù•WÁ?ЬÞe%ž @vLe3`€@:@ºˆ'¿ïøªñ°²?ïöCže[O¿àdïY­¿ßÏËd—Ú'¿çf½+-«¿ïÿõEq#AGNbcu3FGL J0525.8-2014PMN J0525-2010?ïÔû,åý?r
9w?‡?QFåIwµ?MÅ=Å×2?q0°8ãÁ?ndL"ñ™?çH?‡_s¹þAy?d܁fV%?hZžs&u?ˆ‰®°{43?ƒŸò¦áÇ?ïG8uKï?†ÅùÏiä?o1®N‹—?mˆJµ-[?"2»•Í>?"xzCtÀ8?îäÌu‡÷?wl¾Ûw©h?'~öÎ 0?b=(66ë?š'hÝ`¯?r &¯Îی?ï¬)ð›D?w¹Ÿï'-?b}l 	-?V#d€ª?€Vc@A¥?t¿½'õn?î 6 £c?¤ŠJ¸‰>›?|<Û·'Í?½¸^‹
«?¢uŽ	I~?'D¼­X?îØJ­°?ÿ…uñ?YŒìhš²?Ò°ahB? YPy E?‰¡Ë‡ÌiZ?íªVDôë?Œ£:
Âñ?ŽŸ	LW¶?v°Î­å8y?­·èFf_?ˆˆìÖ¶
KAGN4FGL J0525.6-6013?Þµð»-À@ïz€Ïž8À9ۍs©ÏÀ<I<4c´Û@ £‹7?ûìUÿø?³Ãê%"N_?¥x¥X>°j?óo Ä0@?oߋì2?î*æþ§:l¿ä2ì@Ûgo¿ÞT"f¬‡¿ÐÍzÝð,¿â•†¢Z2¿¬éÏ£'7AGNbcu3FGL J0525.6-6013SUMSS J052542-601341?ïÕæ³ËŠ?gÑS㸑Î??…fkJÏþ?.ž€à8¨I?sO¢:Œ?fÃ9""ü?ï²@'ž¶?}ـ\Ú="?SÄYqB…ß?Záw1mhí?€÷jãTIî?y]]öÂk?ïu«ˆëˆ?wüP­÷?eÈâA´|?iwù.–?G\}1îŠ?r;$O—?îñ¹9á¼ã?u‡Èý݀l?t~{¥L´?ULBÖ®[?œ©9àüxš?sƘÏF,?嬨RâÐ?wNtýääõ?Sw,—ŧ?C€'Òû&?'ü<'·c?v7™=a?uÀá?"}zp/º?cm¨"-•?råSŠK\ó?™šªávš??'x8R@?îÞî¿T­ñ?‰t"ِvþ?tkq-i?tî$iKˆ?ŸM;覂?†‡ñ"Þ+?íJ5MÈ,?'96?‰DŠw¡f?q:ü&•ä®?²…ÆC&ãr?jãSqAGN4FGL J0525.8-0052¿ê'ÛÖ;F¹À3\‡D,»À9÷Í-DÜ©À<(Y‰QÞ@ÇRŠ¼\@C«Ë]a?À'Xßj3P?Ç¢C÷¦•+@܈皮m@
¯Ò"¢k?ïn¶—b&¿á×]Ÿmn¿ßr5§º¿ßO{hV+¿åýJä)िïñ£µ}AGNbllPMN J0525-0051?ïð_E'7 ?LkßßÇU½?FTSÜ?;Á§ÕyOô?T@ÊñŽvÉ?C×EkœX?ï¯À½ÓhP?€M®£²ÈM?\4hWL?`ú÷øwD?€ŽÍ/—¡?|ZF§Âß?ï˜UB7ï?€È!{?qUåè
@¥?yr@öP÷??¼sXPE?pà QµN‰?îh}˜dÃØ?{.«R–]J?'EÓϘ£?\uä×?¤æ±ƒÓÜ!?zº[ûD?ïàÅdp}?_Z8"0?\ÝBò^"ë?T]"J÷Rc?`ËúAÑE?P]ÄBÅæi?ï
u—íÙ?šì6ìȍ?wÙëÃ!ó?"eâ[J²?˜[HßæÝ?•Íy7Ø?ï5˜œTÆ?¦8ë,T	?€xÛŠ_Ñ?'wÖÃ'/?'~éš+ó?ƒÿ›DTD?렜—7€?–só	%g?—üÆD'??y°EÞ«¤c?¼ûé´¨Øk?•pgvOËAAGN4FGL J0526.1+6318¿áÖæèƗB@.bTæâ!ÉÀ;"®"i›À=u‰ïØk@½"ªú¿ú?þ@ÊËjÍ?Ò¼)œ0¢µ?àÔ}e†l–@
dëVûX@q리§"¿ïÀ	ÿ÷?ïúDÕ&§¿Ì¹¯ä‰¬ç¿Ül±n¢u
¿ïÿ«±Ê?ïön¼v=tAGNbcu3FGL J0526.6+6321GB6 J0526+6317?ï<`kÙŸ?¡äo¯$?Žàðå»Z?"y,甤<?'ô$Mfä?› Ä0F?ï©e""\?¢~¤]†?ƒç¾Šc?Žw8¼L0Œ?•ÖôKŸnM?št'°_]ý?ìí]ÿ¾_?£8—'/s?§(£cý€?›Ph?‡éê?ª|¯bŠ?˜=Ì)¾ß1?ï`ìšÙ›Î?sUÛí¼²?€¾‹ÒïÄ#?dÐ#ד)ß?‡Mp"M?jn)¦/Ë?î'™[$L?¦Áïf9KÏ?¥…éÎæ,š?¥þxXÂ?.U7?Œœ2Üwð?텬žÔ+?µv¸¶°ÏÃ?•I
At;?¢(µK"á¦?­±
¦9?±DęyBŸ?ëjã!¼­	?ª†xÜ~©?®ã¡÷øNÐ? }èmzu?µ7õB‰S?¢áœíªö‹?î1[nO®?²ÜÞ(D?"Ã584é†?€w™?,?£³Ùôg?‹˜;ýZAGN4FGL J0526.2-4830¿ëk`Ô´«À@à‰~™cÀ8QÔâEÀ;Œ½vîsç@ðmBùyÔ@Ï7ûïÐ? ¢òˆÉ×?±)¸
Hx@¾å@a @a v­†?°`Úá7'é¿àúõŸSí¾¿äv^½|¿ã–Ð[͆0¿ç»ÙÊâ¿ç^1¾éà.AGNfsrq3FGL J0526.2-4829PKS 0524-485?ïæUÝà¤?\!®GóÖô?4ÀÉm?(2ìdO?gb– zí?Z¬o"…ö?ïë_óÁ¿d?c}.FìÐÝ?.W…¦¢£í?=Éz˜«?bº"ò‹,T?aWVÍÇì?ï¯"ïW?{¸Ђ@7?Y¹´]Š3?aöê«xŸê?
_âÝ?zyÃJ¥×?ïòò3õ·
??†Á"Ñ.? æ摥æ?	 0GË¡?XÜ6æ‰?>
†0ÉS@?ï»R®ù}/?s•åO½'ø?@?cŒå»G?1Š†1Ð?€']û%€8?s4_›ó?ïýdØz^?šm?B"u$.²j?WÏL5;s?{ÎÞè]Âî?~ÁA£kY?ï.Ë´7Ä?ƒM·r
r?`tÝö¶mI?j€Ø˜3U?"—Œ­m¤?É40›¿?ïáGÚyd?[â-Á3-€?2Õ£+Ö?#­5Q¡Uv?l]"° f¨?ZË­dê÷ÃAGN4FGL J0526.3+2246?éJb…oÀÓÅyò4eÀ:bnŠ!WÀ<–C£Ã¿@!›i}r?ÿœ
Ý©"ã?Æ3–ÛNDÜ?°,¡r´?æ"ÿ[•R@$=Pš¿í®,Ε#é¿ì÷iCy¿ÔDhz<Ý¿à- Qn޿嚌Wè¿ÂèL:wJAGNbcu3FGL J0526.4+2247NVSS J052622+224801?nÐ?¡q½—¶T?KF¯ˆ"ý?@3uP0K?¥§äp+?¡QÞãvÛ?ê¾.g$/?¹¨ä Œ££?[Ï.¾é¼?e{Ó­ÿ?ÄϨ§•Â?¹th…!Q?î@yÿd=†?–¿½F|N ?hp}SƒXç?a
š@2H?ªqX6;À?–/¸A‰é÷?îä›_ŽÓ9?€åîû¯?U"+4Òë®?>üíÚøâ?¡	¨ª–‡?å݇âe?ì	†7MZb?µ`ŸáˆûÐ?\ÃEn-?QuTL©Ã?¿@Á2²&P?µOÍ*$G±?ä:pŠ	a[?Ɔq;àœ?eŒæNœO?y='¤L?×aќ¯?Æ`G¦#?ë[QBpp‰?¨¨Ž…è'?yG SF?qiŽDÁòô?Áȁóyx¬?¨~¤:?ì˜/¯ G?$Khýþ?kF)šW)?^gŽš8+:?ºeÌ֐x'?MþÏAGN4FGL J0526.7-1519¿àâZ‡NØÀ9~ÓØYÈÉÀ:d)uDÀ<FøE ›@Ý7•B?ýçOšr®?¾öڒ]:?ÁiíˆQ@ÅlC9@֌W¼ªk?ïÿÐ/WÜ`?Ö~?¶N[¿Øò°¡ôó¿àkÑtÒ9ô¿èŸÑâ5iÄ¿ÇE"/_iAGNbcuNVSS J052645-151900?Ú佄?ŒÊ™©¥N…?b¶7DDêt?aò´'q'?ˆ§{"…¶8?‹ª]%
ðG?îãŒPþ¾?•æM¸€Ë©?"Ü	
–'?"Ú'žízô?™ qX•"é?ŽLôèYL ?î14>ñ?›á˜!N£?@7±$Ù1?Œ£l&$õ?¥œ°'?•ºÈW6š?ìÖu#‡]q?ˆ«dÜÉP3?ž‡Š'ª¡¦?wÑWå³è>?±ªtZH_?"ì{\Ðb?îÚámÌ>æ?–à¢Mºvs?†ns€IIG?‡‡Ñ>MLø?™l˜‰Ã™?'@ËXJÈ:?í¸ÉÏ[6?®ÖRÅeI?—‰ìñÜ?«×Ú~"?±/øuX?¦0;#pH?í+@<¨tJ?¢~L‰‹þ}?š@â^²À?–Là¦á?°řd°þ?š»òVk"ï?é@­³Î?žÓ."°{?¬úº³
Â?Žþ)*	®?ÿ=œ\†X?™ã=0ÊØAGN4FGL J0527.3-6223?°ɟéiÀ@ÀœÜD9À;ÝùzªÁ	À<ý'œüûi@!ûÛ® ?ýç"Ä!?еâlvK?uÁ	þB?°ÌáßGgŒ?òBxåÄë¿ïþ×áÓÅ?ïÿJbú¡¿æk´ÿ{ µ¿Ô…4‡Ç	>¿äŸùš‹1!¿®$æ¿<@xAGNbcuPMN J0527-6225?ïÛhPÌKH?j.ÚJ2?1ê³?è°?*؟'Dòa?q:xõPÎË?iBí¬;–?ï"ézÇ5M?‡£ˆøåï?bL£'Õ	œ?h°EsÞø?Š2x'…œ[?ƒâ@AX£Ò?ï5Í8ÏÍ?Ž§Šm÷?h=ߌªŒH?pË<o½+?™1Šc1,è?‡UÑ(N?î̵c,RÍ?"H"Ù•Vð?wÖt2T ?`æ~œ¹™Ê? 9ÛCã"²?ƒòúiŠØ?ïɇ<—?rGUÑ,%Í?>¤šqý:?<VVü07F?yRýˆ8—?qꈤ¼f?î8W'ìŠ?¦¥áû
?pIꛇ?vÀŽâÇ?¤ó=/"'×?¥ûz–;n«?î¶Ô°pö?'µä¯ÀÃ?nQkˆ\Uü?r¡V§®'˜?¢­žBҋÉ?ï¤oìü?ìŒT£±?¡|jãz?ŒGôÁƒO?q{V±<K?¸o'Ž?¡_[j•è8AGN4FGL J0528.7-5920¿á¶5ü¼(»À@ĝàP7PÀ:~Æ/#ÚÀ<¢Û2Ál@|1~Ó?ÿþí+%Â?¿€®¼šq?­rp#ÃBy?ñ¨—³æKú@…žß(Äð¿êº ¸\R¿Á+m—C¿äOc 8o2¿Û¢"#揿×è÷»7ùì¿ëëgÝ^ëHAGNbll3FGL J0529.2-59171RXS J052846.9-592000?ï䤌ç¯|?Uî"ºøµ?<Â!V–Ï°?*ùxŽ€'?gÃ.ò"|:?T=w̖¤M?ïØ64ÅY'?rßÖlAG?:_o<b"N?Cÿ"¡ç#A?r>îÙ"?p¸ •'?5?ï˜êfÝüí?oñ,âèì3?W§QÂ-J0?Tg(øH?†Ð|lç~?mm"óØÚ?ï½í9Ÿ?Z?DIj1?Oøi™ÝÈY?1"ðï݇™?}
hYÌ?Y{Õ¼Ê#?ïÀx–Ó?nõ—µ«€q?Q©"+Õ<¦?A2ó33?{YPÃË)?lÉfÎY¬|?ïs|è?¯E@¸?L¥×‹ðZÍ?YÏhÖ~·?¸a¾ˆ|Á?ŽÓgSrÚ?ïFX'EðÙ?€}³™#ïË?aELhÍï™?Q>qt¢?•D+ßôö?P%­q¼S?ïLüOÚ?y"|8¸?d¬§ZM܈?R¥!ÿ+‰9?"Êá3bã7?wàVˆH¡AGN4FGL J0529.1-0101¿ïût{/©ÄÀ2¸Å¸ÜUÀ:'ËÌòŒzÀ<#WóÝ@åü¤«Æm@'Èš8%
?Ýhüopü?Û*à~Zxò@0…ÔÀ·?ù|*­þ€y¿Ýpõ³ ?ïzËx8ö¿ç§¬_nû¿ë+$Á€hp¿Âðvà‡Û¿ï|þyØAGNbcuPMN J0529-0058?í£œMÊÎ?»/vä/a?—-aPì›c?¶'¾ C"Æ?ª/ŠˆäÓo?®{ÑÀN$«?íÝûžF|'?´ÝPÁx*À?Ÿ)¨!Â?©'Â+wìº?¢‹ºÄó ²?«Eې
Ùá?ê— ä.ÆÅ?ªKäIµ
?®a0Ɨ4­? Q¯öʚ?¼`zÐ;þ?¤u©h%p?è‡Sz•6L?¬(¡$vƒŸ?±=…? uJ'œæ…?Å^©÷"R‹?§øŸ
¡Ô&?ìgß?³sôœÀ›?Ÿúë™Ò? Ü_+¨B?³•M.Cû§?®u"áWœ•?è|.q#ü?Éx•x!Ð?Á+€cŠ
}?Ä7S–ïµ?¹Ç‹´Ž?ºp+C+Ò?è®»°«ë?­û/	þ'Š?µãÝ֚M?£¶½ù—¨u?ÂS"¸wçS?¦p/Lz«8?ÝF¹™®?º¥Œº]è?Àl00Z¡ó?¸0O16Eò?ڃÑ-& H?¿'¥©zë·AGN4FGL J0529.1+0935?ïYÎìØÀ*Ú ¼8*À:&ä›ök,À<[}Ë@ C~Öʧ"@†‹ýϤ?¼x‹×åп…aC^EýÞ?Ëxëä•{@gmrU?á5žÎ^¿Ú>(¤äÑP¿èQxbè,¥¿á8Ï>ìúÀ¿Î/~Ȳ῿áå]‡š"•AGNbcu3FGL J0529.1+0933GB6 J0529+0934?ï¾\j C?q§¼g¼â%?H	8€W?8¥ìhŠ¯q?}Шz6?Á?p»Õ%+¡?ïÄ5Ê^«?'q+«èñ?B\-Ã¨?Jij˜k'­?{¬â)æ?Óso
gI?ï[žnH?ŠÅH®vsÅ?dnþ²Å\
?R7§r']?š¬l…r?Šr5¤?ï;S ʌ?pA(fíõ?Z3HÔõƒ,?@w\Ð1þw?–ògS/Ù¶?oäߜÁïà?ïD™Ž °ÿ?Œ÷ÑwX?aÎÛqå?UžU¾"?•3—Có?Šo1¬>.?ïlƒÕü»?•Ôgà^Ûö?NNèÌ^§?[À¿¶§…?'~òÈ`¶·?"éè%=³1?í«¢'÷@¿? a皑8?u—(‹ò?i—vt¡ ?±Iyf`k¬?ŸñäíU?íÀå&ϑg?Ž}hTŠîF?sY¸—'?bMô£U-"?°Ã;@­K&?Ž¹Ñ³ÁùAGN4FGL J0529.3-7243?Þ'XúºhÀ?à.D¶é6À:YDéN
À<Q+"€ä@mÑ Ç
k@™µc#»Ç?À*ZÜð[r?±:ÂÇ;=?ñ4+
oÆ@4"Y8«m?ÛL»ð[¿×cL@Í¿èd^y]¿Ý"Âãü¿è˧¾uq¿äm´8PÍAGNbcu3FGL J0529.8-7242PKS 0530-727?ïñùWlc?KüläG·é?8_ghQ§?0h;ÞÁè?VúRõxñ?FfÓ6†ïZ?ïé.]6×?h±eµº?1ˆë/T—ý?A†éU7û?d â&
ûR?ešF%ò?ï¸Tã1=:?snî0Ýà÷?Y	Ú
@õ?b}Bb\?}"Ý1íæ?pЕ>Îs?ïàx§ËOc?KÞú9?@b»»rQj? 'ÎïÄK?kn©¹€å?K€â½-eÚ?ïäðÖ—?`R;Sk¡Š?L9i Ö8¤?E";#"?dÏMM˜<?Z³âqþï?ﷆnf'?Ü¶ŒÐ'?@"eŸl\Ý?VÊϘÃT?
f:9?€yD²à5?ïã\þ€?~_jþäh?ee—WI»Ô?mÞ_E±¢;?‡_aSEç?y±'ôÝ|8?ï¦Héþ¶Õ?hÉ͹e͞?YX´R©¯_?AX‰	ÈÞ¨?ƒB®õM(æ?gµ`úŠ­ëAGN4FGL J0529.4-0521?âÀ;vp5À4§"BAÃðÀ:	"V!uÀ;Údµ—&@'»Ÿ}ß)@E&z¾@?Èi
!A?Ñøá}³à@)=Ùb·@´Ž®¯?ÈqȨü¿ä®Á~ºñ¿ço£üÉë¿ë#3 hÖ-¿åù)Í¿ïîäŸQiAGNfsrqPMN J0529-0519?ïŽ×±'C'?¡<^17?qügÇrñh?¡瑛´¬?ƒKß²ºð?zÆCy¢?îÏ¢Ôo6?œX{ù[Ý?Œ"5V£ü?Œ"?™=Á;?—ý[ZУJ?•½¥<þ:?íf,Ÿ›;Z?œîOéŠÖ?"ZD|Ù0?ŠP€#xÀ?¯ÕˆâVÆ?—È·ÚKÞ?ëćþUtÀ?Ž,¤FócÍ?¡cKS
u?{RbyÐ?¹*d=ñ?Œ¬îŽ},?îv6+qY? ‡Ë´æ"?"©4˜î5ï?E[{Y?£rP +ê?ÇßR5'?ëðLψá?¸âbnsËá?¬îš¯?²)§ç?²(K™H ?­¥ Ùô?é'n²*W?ªúnÓiÁ\?©˜:Þsx?˜ݨ"q~?Äü8ÜP´Š?§Šªuz?äM(¶Ç@¶?¤Úô²éG?¸ê§€Çl?›4=/œŒ?Ñ+²ä°?¤î =ŠAGN4FGL J0530.9+1332¿îÊ`UL°À&YWŠ*'À8Œ×òš½À;={á!îg@%C"d(I@­
?#?­êYXR…?ÑÅ9$ä»×@¤
COàé@0à?ÊN½þ'㟿Ûé
_¹ùá¿èVݲME¿é55¬E¿íàpÀ¿Ý,_#ÑìFAGNFSRQ3FGL J0530.8+1330PKS 0528+134?ëJq0"?ÂGî©ôä!?Á¸ÂSÍ?ÁdÈ÷Þ§?—0ølú†?£'ôn†ä?ï†ÑÓZG?˜à.R¯Õ?fÉvy'¼?z¸'Ú–?ˆ™-¤X-v?•~WwIÞQ?åþ/¾"?´ÉËV'Bn?Ë{¦ÈöQ?±;¿¯@?¹pòØæf?¦Ý)/'M?î¤Eµtt$?‰0¥<Ϗ?^1U6å?nð³µèBi?¡dTöׁ?…]Î)}®«?êï=Ô¼?ÀPRênÚ?Ã~e….ÂO?½àH™e°ù?¡ÔšôÓö?ŸÅZM¼<?îŸ4zIáå?³Gä:µ?ˆbë€Ã¿? sëäXôR?ŸçúòòGÓ?¯pØxZ7b?ãtyÏyÐQ?µ{v¶??Ò)ƒôŽ)E?³adN•+¤?»¶!±øØf?§dîåM¨?ê¹jÚ5ã^?ª>&óˆ*?£[œÙ¡
Û?'|qþeš?ÀCmaœ?¦ý¥9ÓAGN4FGL J0532.0-4827¿ë)H3~XÀ@fýüÁrÀ8;u!MÀ;g¤(hÔÖ@]
È°ÞZ@±ƒ›*"R?žTþ£Î?­?³è'¦
k>@c5X§a@ 
2~,€¼¿Ðëæ£7¨
¿Û@.Ä8©•¿âËcÁ'ý¿â[Kµà÷ý¿å6±'n"ÿê^òԞAGNBLL3FGL J0532.0-4827PMN J0531-4827?ïæ…^_m	?Yx~]-ü?<ìÐ÷ºáª?/±*‹Ã
?eÝK.—º?WQõ8üHÚ?ï鬖mâ~?g©qbǍ?1æóòâ'?BnÓعp?d‹'&Â?e|hH?ï²½}µž™?~¾þy^bü?a¥?5Û?rqܾnP?}ю‡¤?y˜Ï­?ïúÏrª¨œ?07ªá¬Ë>øÜdC?ç>ìÊý¶kq?CüçTŒ€?/¸!]xê†?ïÔ»j0î?h"{	Rž?9àJÙI?0H—ötT7?t©ÐÐë?geà¬?ï¾²‡!i?"¨ç•P×?M;b•ÌçI?jKJ}f?|ÿP"Z!?ƒA_‹ Æ€?ïŒð?‡n8?‹?Bÿç¨Ý?hMÛñÓûi?vؾ|ÔC?†°yŸ¯=?‡zÊ3…â"?ïó"ˆsè–?MÉ²&
O?:¡"0L?÷!×áI??Wþ=T>±š?M²…›ÜOAGN4FGL J0532.6+0732¿ÞQ_½À+uîÇÉXÀ7"ñÓ'éÀ;B™Øƒº4@äÄ*;è¹@ž{€©ß?—w¾8Ɓ??¸
Xs‰@-š
^ÿ@kß/ûÆ5¿Âç<9¿áyÛX€Ê–¿åô>‹$¿äN'ÿú ÿéÂ}h‹…¿í*7/AGNFSRQ3FGL J0532.7+0732OG 050?ïÆ×1wÓ?n唦ä?S0¬¨Â
?Oy·:Õ5?wÈfÆ•æ?jÕgŸ"Nò?ïºfܨÒ?†ðýÿÍ?U긲õ±?kƒÿ]~šj?}RBò͔?"¨Ä»?ïÀ/^×¾?yp¹ûµª´?cgkwÞåÿ?m3©€ƒ?v4šëÃýÚ?u{‡ ËÐ?ï§ÙZ¸D?iÊLÙ9O'?c4ó³[¯?PÂh¯fÁr?C¯ì
"1?d¥Ù¢ÙîM?ïŽP_`Z*?Ž¿DÔ¾Y?Yî+£'$?U`ÅH¼4ä?‰."¨ ›?€jöH:93?ïZ&§ø"?ž4fÄB*@?nŽÙñ$OS?}dɵ!R?éaÓ»›¥?œJN
Ú?ïÀÅK½Ý`?{IXJ!ë?g}"Ö¢?t¯­Ú$Ã?sÞЂQe?s¼Ukw^e?ï*íGÁ‹?ƒU{'nW?w%Ã*ÿ^?g=#xo^?"ô=¡mšÛ?€(Úm3AGN4FGL J0532.8-3941?îî4/ÝÀ?p‡¨ÖMÀ9¦Àð¸,À<]sWN›@¯B¼I@hÀ³¹Ö?°°"Üj ?¢ÊîË	K?ì•Õ>á<F@
£	Õk׿¿ß^TùM¿äÀVìÔª¿è¡Ü>ñ§¿èáyaë­c¿ßúþÄÄ
¿æïËoÌÂAGNbcu3FGL J0533.0-3939PKS 0531-397?ïúëUó?A–™²Ñ	÷?ðÇóÝ?"Xá'?AU˦–‰?;[{gޘH?ïèŠw*?hVaªwµ?1¶Å†Q?>"ŒP¶G?eTùñŽô2?e³€È­s?ïÀš‹[ø?f
UY#ãÚ?R£×~_?:'O/ò‰(?{-'¾šä)?ea½²?ïô…ˆ?9X'œK?6$Ye¯? G-Ó?Qn2çù˜ò?5g_6FÞ6?ïõYkߪ©?L'^S	è%?$îac̸?:j*I?R¯\ ©&)?I–'²Ü[?ï±Ë$^·¤?«E0"H*?@´ncqæ?KþÛÖæ@?'"¿?€ßU÷ì}È?ïŠsU¯Z?yžj§ÔEî?]Ó;cá?R(ÞOéè¶?‰¨Ã}]t?xMX'n?ïà[ïXס?Xöo³l(?P¯í)0Ì?A×`ælmñ?gLŠ8îƒ?UMސ/ÁÆAGN4FGL J0532.9-8325?ë"oIu%,À='xÝao‡À:ž‹¦'Ï¡À<Z›•\W@ ceù"ð@$á{°z‡?ĨèÁõÙ6?½š¸}ŠoZ?øNbS—@·ww°»Ÿ¿Ù‰§^(T]¿çv•žoû¿äêÖù¿ß ¾Q	¿ã~ÛþZ¿âÿ90£6AGNfsrq3FGL J0533.6-8323PKS 0541-834?ïùâ*½?6±ÔØ
6?‰Æ+ÅÀ|?•Žôhó?GW?ÈϚ?5E>'ê?ïê?ÞV%ë?hžV7/DN?)W+¦¶vÜ?:—ø¾œ€?d*¯
A¯"?f^qNÈ¢2?ï»·v×ÖI?s.á 6š?JJxûm#?3Ü!~?~ÛÓð†©?sB\ŒÄ?ïÛ&`€¸?XѺvv½k?*7¹DæC?•W'›)4?q›ÎåYú?XÓç©1f?ïö0óµ;X?F2™FGH?¨?©ÆvW?Ø&a­ø°?Q£"µPN¸?D˜L83§ü?ï´ôƕH?'ÅÖŒš?B®×›Q?T²Ñ!eîV?¡Ã,7²ô?o›ØÞßç?<G?wƒ
í?Sé&å¿?Bx$žp3?‰÷_6m?wC«"ƒ†8?ùÚ›?wxîùÿR4?C먆ô×ø?5×9¸?Æø$þã?wrð¼ƒçöAGN4FGL J0533.0-8446¿Û'Ð+ځõÀ<Ädf±åÁÀ;g
ÑZÀ<…ÚcŽDÒ@ùX¾2*J@œÈ='?É<;±î?­Ø°A ?Þb§Êà@ÅÌ8þ#\¿ÊEŸœh?À÷ö†¯‡¿ã{Âîýy=¿ègÍ<^¿ÒÞI¡ßŽE¿ïõ£ñpwAGNbcuPMN J0532-8447?ïîÌ«·ß?RŠØe!6ð?y&»ƒ'?ÙhÜh?`?ŠöÚ÷?R;1© ?ïâ
^7mÕ?nQ;bÕØÒ?1.Ü¡H?;.9b1qÚ?kÌÆ'¦<?l~8ڄøÐ?ŒÎQ?wåxwƒ±?S îF¼?B±ìoJK?‡ù¾ÿKþp?w‡–&g?ïØýØ»öï?SŽ?[¨"?)nÈK0<Å?ƒpˆÂ¿?rµmÓ?RðæÝ;g?ïØ·JÉ@À?hÁn¶•?2sŠVÊ?%ˆÇôÜwK?r"\"¨?h2Õèæµ?ï'lÄîæ?ŠËsKö$i?IãÙ&J6?d6wºSP?Š'[àæ?ˆ×†²‡?ï>
È{À?‡[±n´?[¥šŽD£?Z,¢Y3ˆ?–Ä 4f°?‡RiÓZý?° !f?sÈ,‹m–º?A4;('Ãü?6ÌíVlÛ?ÊPDÖh?sºn [ÿAGN4FGL J0533.1-6119?ï†<%†]ŽÀ@s(bõ˜žÀ:¨`"†ÉÀ<bûáN2@õÉe²@à´Zåÿ¤?Ì&ñ[wu?Çö?¨·o?ó	7KƧð?ïücÍÒ'Í¿ÕÙ6ýîü¿êBjۖ"¿ìÂ¥â'Qþ¿æ_Ë‹«D¿ïúè3Z `¿çb¿è¸¼AGNbcuMRC 0534-613A?î¾Îâ8l?Áþ=)úó?¢  [&V?Â
'@ë¿?o/hÎíÜ?wÌÇÌK?íñ˜Æ$?ªž·']M)?šHtºœ[†? ¶«³ÏÊ?£Ê\¡þ?œ&—•ô£Ÿ?íٌ£½? Bfê¶:ç?˜gU碗î?'A6¾ôk#?©ûgt@_:?šCñOÅm?íïNÀ¾‡Ì?"h»{!я?£…«ø'7q?0T$¨''?›
Ïúš3Ÿ?}•
ӕC?ï-ôY{è?²r!AA‰z?•YŽ­ˆ?²a0p°ù$?s¡¢ö9U«?y_úIZ¯?éÀ'+ç?Åg~S0C?·{ÄoÑ·?¿㶷üJ?Às?ÕOtª?¹Ä²G̃?ìÐŒ¿bù?¡Þeìçöÿ?Ÿè×3G?—sµ‡Ëa?±…½×'¢?]â#ð!?é­ýèù?²QÅmӅ2?¿^0îÛ¸?°(…X!²¶?³9Ç< 4?žôÇÆ:"AGN4FGL J0533.3-5549?ïÛzBÍk>À@}Š2ôIÀ:')óÀ<rfàß©H@ý܌ˆd@£!ØG?вLBù¤Ç?ÕRåB˜?ÿ0ÈÚÏÄÏ@rßÆ?é¼|±¯¿æ_(뱔¿è'm{-ž¿ìâô÷ŽAw¿æ©Q2!»<¿ïÿ°NçÄ AGNbcuPMN J0533-5549?ïÄI¬­ƒÂ?vò4Ãߛå?ZOÿ­ä?Vø
Þiÿ?wG*o" ?s!W©5I2?ï'qhD"a?'Ä&BÜ^ë?{jY ë?€ú…Q?#?"M¸måζ?‰i3œ"˜?îYO£<–Å?˜½á;]'ò?NÚñ'o?‰eMŠíòF?£O‡ÆÔ?"iR¤É•¹?îã«#bcU?x®£$0ƒ¥?†ÀSˆ6q‹?f&lf?˜*qÍàŽš?t=rÛÔ.?ïfƒü	·u?ŒÅwtÔÞ×?i\ôZ!i?g,xSÚºÐ?áöz|:?‰–³öœF?í`'³?«ÑXíiëÐ?"@Áþ?›ÍsÌ?÷?¯·>ºã±º?¤Q{‡Z³È?í ÂL™¨? S^\?˜ª83߯?Qò¯î_?°Ï_' yS?›¶ýIK?ì¢9¤¢`?"Ô­Ø&Õ?Ÿn®sW?†¤R2¼e­?³&—.rh¯?'²SŒµ~©AGN4FGL J0533.3+4823?×Vršs«–@ {z_A®÷À8t7	‰À;ˆ"/•ð@ï-Ì­B@–n^'lV?T뱤í?¶./g5Ä@øDIÛì@Ðw€üj¿¢ÞAbd¾¿á›CRe'¢¿åÉ(½äQ¤¿å¿˜f"²Ð¿è§ÂòXw¿ëô—ìñ/ƒAGNfsrq3FGL J0533.2+4822TXS 0529+483?ïhj…?†8ï–Ã~Ú?[º"b+Ÿ?Qâ˖0Îh?'AI¦†å?…,¡á¡!!?ïJ?[W!? <R‹{b?a
É'é?i˜Q¬?"–»x#˜°?ŸÀ÷7¡°S?ï'Ü:ËOl?'7~'ÉC?fQ8²D$Ž?p~å•Ý?…ô£Ӊû?}Îۇ0#Ÿ?1Ï(zP?^p³*}?eD}N²…?Jé^цc?w0ö1;Ÿ?W$AáËYT?îųAÐÔ?š¦"oavb?YqÍâFg¶?P®eë©Ë?¢Ù=qÆ.?še¢ ðê?îv|×f[?±I°ø?v­0€uŽ&?ŠãF(1?¥Â²h?°´ƒ'ÓoÙ?J½4÷?†	hÛ÷è"?l¸ô8¹m?töª¨÷æÅ?‡m04D8?'"£	Š»?ïZÊäÐ?{O°Œc?zá|äW…?hâÃn°?‹Üˆ…ãµ?t®‡*îÎzAGN4FGL J0533.8-3749¿æo¾*üÀ>ÜÊ>}QÀ:¬6ÉÀ¨ÒÀ<šq
"=@ba§ºÄ@m(<_+à?ÅôšÇ)?ÃCOàèã"?çÐ*_z@ ›'
`?ïôb¦h_¿èuüÜ_¿ßéÔ¯ð4¿ëƒB‹?å¿åÇ-†K<¿'üyº´¥AGNfsrq3FGL J0533.8-3754PKS 0532-378?ë%½
?Õ¥éQEu‰?Â×N'wµ'?Õ¯€iFô?r7°œ½¥?›jã>Lm¡?ï¿m…¶Û?wÖ¨Š>Ý?Lc'¶­+Ê?S—æ4«™þ?|¼Ê­Ú	ž?t–ÅSÜ¡?ï-i'T?…C¸~›˜K?rI›9_Ò¸?~¨8¤$w°?‡ØD¢?z\¼p?ïԎŸaüí?SôF£§^Y?DŸØ	#‡í?'ž$Îxº?s$µ/ŽñE?S-§¬æ€?ﱪ~r?™Ÿ`³b?nˆê"gìo?—œeÚXU?wæˆnÓº(?€‰÷\ç»Q?ï9óÊùl?›aJ<?_<÷w†Lr?p\ˆSb‰?–ÍÀJ"ôÌ?™ t!,N?ï#ˆ×?ŒCŽT~øÓ?yŽÞÚe?'Üúù)?•GÙªÎÆ?"Ï2V[°?ïo;Z&Ś?tþ:Z}O»?\"L£¾¤?If€yàñÍ?O_òUˆÎ?t"¾C6©gAGN4FGL J0536.0-2754?é£îCøÈÀ;ÝCá`xÀ:ß9á£À<]HœQÿ@·FŽ"½"@Õ¶€Z-?Ëîc cbP?©sŠd§?ÖÏþ…Š@–ˆ¼|ž?î10Ÿ//ÿ箅^¤%9¿æÓZ»7y¿å·Š`@²x¿â¼(Fp'¿ïÿËA²Q÷AGNbcu3FGL J0535.6-2749PMN J0535-2751?ïÑÿià¡ô?mè¶Ôe7?A˃½q?3"!')ïg?tà1°àˆÅ?lX	}îrƒ?ï´°ùT½?zŽ‡²ÞY}?RÛ؃Öa?ZÐÞãþR8?€x]­"Ûæ?v3dÍk?ï[‹Âý|S?®-L®Í:?d²H‹Óð?jg{í–?'ø>"Ú*?}ƒ¥p…?ï­ðU_z[?\þ'	V¬9?PƒÐúläÎ?1ª4"6G?'sp£@ˆ?[Ä%Œié?ïqqúÄ+é?‰³cu­¿?SþbqfV?Hkuf/?'ÚwI&~?ˆË0mð™<?ï9á+î4??']%‰¢6¾?_¦¥'i÷?jû˜,Ö#˜?–Ép9j?»rD[·?î¢Ôld"d?'¤ÍÞ?t3 í"'?s!À~韫?£LU<÷?R‰wµ?ï
ælûÝ?{±­ÀÉ?ebGŠŒµ?Qm'[¾-?›–éˆf¸¾?zqÉÙãPAGN4FGL J0536.2+1733?ïÞ´D&ßÀ5çB™Ø"À:Fêóÿ@½À<eO1Ì@}4‰¢?þFÙóü¼?¢4GÛ5ñ?Οÿº4ï¡@ÃÔ»®—X@Jæº3Âû¿ïþR`Ÿýâ?ïýýu‹r¿ÏëŽÄS‡¿á9‹Â@Ð¿ä,õÌ W#¿ëþ? ÿ¿hAGNbllTXS 0533+175?î²ÂӂQ1?›šäҏõÐ?xÒ,[s[Q?rÆØÊ7˜\?¡¹;"§?˜±ŠÚ—™B?쁭"Ò+Ë?·²•-E«?r|¡ô)…§?­è4¢$?ºÊÌÊüñ‹?¶srg¡Zö?í¿¼ÏÄ?™'Æ©Ÿü?ŠÛû·n?"Ì:l¿ÿ?­MA1«:?•SÜ4®9?í¿Íw'æ?"0{P‹ç2?‹Ö´PUã?h£`­ìò?­–äSÞ?·Â˜!9®?ëù9IÍ©l?³3¯Àò§?–šCy»Ê?ƒÔð¹N?º¤Òvž²?±2ùµ¢´?ç¼øà®4?Æ»æ¥;
?""}ÔUÒü?"Ô<8ݚ?ÏÂØnãÁ?Æ2ÂàdÚ?éé¨ÆïNh?¬a_]¶ÿ?¥Ä¯Íܘý?—ì
z¢?Âè0ð&²á?§µ²ªˆ?ë\×%¸˜°?H"n?™HÌôT5?ð2¶kKz?¾ÇǪpy?škÁXË)QAGN4FGL J0536.4-3401?ïL›G!ZKÀ=}Š2ôIÀ8¡è
šó6À;Ý6'Ú9@©½H@û0<Þ­ ?¦'a;Ú È?µ'ƒ§"Ùì@í'ÞkZÂ@/cê¶Ó¿Ø6µž²Þ¿âÏi)Eƒ¿éY£àDxÖ¿æÖ_îÉ¿ïCB	[¿ïÿ²vìAGNfsrqPKS 0534-340?ïõ]‹?E³8†øí›?;+ÕÖï"?1¸má"q?N ÙÊáî?@'ìtµÎÔ?ïæ38Uv?k!"Ï.i³?5
8?E±Å´<é÷?gOKmÂËI?h-Ie‹?"ã•ø?"OýN¸à]?púTjF?x‡ð¸°ÿE?ƒVM …€?€PPÀƒÞ‡?ïû¾{6"K?&ˆ0¹ãx?ª–Ìjár?©¥jO¥?:aƒ7<`?"Ù]Çʀ½?ïð®A$<?P :,ot?D)ƒ³Å ¹?=7W‰ñ‡J?TŽ»ãÿ
?H…*Ì(?ï´m	î–K?‡¾'|m¶?MËE|:h?fD×dD<	?	6ÔF?…›5+?ï7–‹å?ÛˆkµÉ?uÉ·=VÕ?{Ñd)&í?"šÀ¼èÊ?Qa­	²?ï÷‰9?@½&úÄ×?0FŸ/
D ?%0ƒ^³ÿ?I¸O"#?;´Ê÷æ*õAGN4FGL J0536.4-3343?ëŒüÀãèüÀ=h"ƒ‡ß]À9L&ÉÀ;ÏÏò=@!‡	^Ú+?ú|Y¸:m?´âlFOD·?»rØ Ñ­m@
pÇZ@©U¯	¿ÙZÿ**¿¿è֞b+CP¿Ñ'd@ò8—¿ÛúcWh¿×?d"cýV¿Ð"c:AGNbll1RXS J053629.4-334302?ïj̹êÙ?»8 ¹é=?7N0¼t'?1'Ï"ð'?'IC>8âÚ?»:,ª5¦´?ï¨ÑAÈï•?ÐÉb0`?XÏ?š'´?`»Q.V¹¥?'±Ç'@(ù?~ö‹VÇ¢??îÙìDƒ´ø?"º0áößÙ?^'P'U¢?eJ)o</P?¡l©5=Ûu?"»«"
A?íGŽÚxÜá?)DqÄÉ?vu0Ék'Q?\ì.´*?´\6!O0?Ž½(/˜Ñ?ïv-<_h?"V:*e‡®?S¦ÞÄ ¡Ð?N—²nf·Ý?ÿÕ «Œ?"ðÛ¡†?îÁÄæé?§F¬þúg'?yo§à0»4?™ÞPá? Àn±ÃÄ×?žnà'Ù†?í§¤à'P/?¢Xü±Ç?gaÀÛñª?k_…eËÜñ?²ÊõÖ21?¡åÿón6?éÅÎ"­?§Å.°³
?‰
—à;Q€?xnqä¨'?Ê(?J~åt?§8Ñ^«AGN4FGL J0536.5-2548¿îØi ˆ"À;Á?ÐÐhÀ:òÚ¬‰`fÀ<¦"Òb8@ 8»*
Ä?ûî[ãU¥N?Ç.DáÜS?Ãí†*Ñæ?üÉåvç½ê?üku.€F¿ìðdaS'?ïâèÍ´SY?É.Êî¦;i¿â5Z 	 =¿ÛrMºÈé=¿ÝïN¢$'–AGNbcuGALEXASC J053626.90-254747.9?ïÒ[s´`?dûXºü÷ª?C'#ëöh?=Šìá¥W?tqii›
.?c©ÇWv˜;?ïš>BB4?ƒf;®	ó´?^
JSPÙ
?`yík?…®ÓØþ¶?ïÐ[?ïxÊV¥Ô?wa›Ž®ßr?bMß
)ã?_èWéà&Æ?9ò•eT?uR±/¼Ëî?îw(‹Âôå?'+ô!êÔQ?x¨ð÷dü?b]Sâ½h?¥xY@Ù§
?€ÖQˆAX>?ZŠ\‡?wòÆ!<?]^1´¼|?R4OU"?"scc7?v8aùÈ?îã/ÀÎ?˜O…('S&?q®;Üù?xíÔã¬?Ÿ.L˜þÍ?•¤\(:Ú?ïúê[Aß?"ËÒ,ÜLµ?kb
¦=?hù4Or?™Ÿök[â?ƒC'+(û´?ì·gc¢¢é?™Ð@W Ä?'fO™(?u‰ü0?·÷úîù;x?˜ÙÓ¼WAGN4FGL J0537.7-5717¿µ½5þÈ%&À@2'!%¶À:/Pž~éÀ<}`Z³«@ñ:ǧ?ý~"_¦XÅ?ÁÁ¹my?ÆBº$Sœ_@w´_½Œ@j/š¢X/?ïÉ­}ÒÝ¿æÙäãD¿Õë&>®Ÿ¿ÜèÿI Û¿ãèZ&½+¿æDiò!vAGNbll3FGL J0537.4-57171RXS J053749.3-571844?ïÌ¡^4×?ri-·"å?Q ¦‡€?D¦Ñvß	z?uG'aìD?qÔIÕùQ©?ïwVFÄƪ?"·Á¿Þ?f¥5Ëë-¼?e»C‹Œ?Œ ÕLH?")œ×Å?ïkâõu?€H=˃qÈ?g˜ÅJ­¼Q?bTGù"}>?!M*ö»Ã?~9_I Ì?î´*¢ýØ?tè<Î=>h?Ô†d›š?\KC"µ? H44*£?rS=A7ƒ~?ïœn|¤/9?zT[3óƍ?k*-5ýAÒ?b@ƒëæ?'ՄMwm?v¤/s¯Õé?îoügÍ¢=? 8 ¶g‡X?zRËöÕg?€gíÅ­Ù?¥µà6Åz?›äÒ{X(?îÚϕ0Ë?Ž-l¼Ü?~ürÃË((?~"ðÖÚ?œæð–Sߓ?‡	R'ˆ©?ìÀõgu?¸Ý㒺l?""𻁅?vØñ¦ÕÓ?µ3Œ/µg?ŒG/wAGN4FGL J0538.2-3910?êN€e.ò¡À>LøŠ/À:îäŸQiÀ<­C³³÷@ ͪÃ7£?þS#ä
Öô?ÄUaÆÄu?±ÞfRDp?îªõÂ9uí@}
yæ ¿î˜×'2tÇ?ïömzVÞ3¿Ø70£‹àÉ¿Ý;êý9|#¿ã2½ÂmοÜl+Â{AGNbll3FGL J0538.4-3909NVSS J053810-390844?ïü;àß[ù?)€²‹kÂ?
"h|cF>ÿ†"´ª?:|«%Íää?'t5°½‰­?ïé9Àý?g÷ŠðoMp?/1\át>?;apò³ÿe?dÎL×àÁ?elvwâÙä?ïÅ_yH|'?aü¶›œKû?LŐ½‡Ÿ?6š@ðúkN?y·Ÿ5P?`õßñdØ,?ïääRaö?EUÄÉ×ä7?9y¶ÿ"s?®¯¢SB´?gìO½ç/?DVVuˆ?ïùÑMm¤§?6Ú=¦R£?$æ´}¦?¹äí+€ã?C¹Ð8çÉ:?2ðã\ý C?ï¸!?…ÁŒ(¢'?>¬SþK—s?P¹RŽ?Õ$—p?"øä½5Sj?ï©'³ð?m9÷â>ø?Sdõ6É ã?G{"Ö4êÔ?ƒQŸ–ɹ?k	hgB?ïÀn`
h?b®¢<šØæ?H²`|Èç?5¬jŽ¥ùS?|²ƒÐ •ª?b€'‰ÊbAGN4FGL J0538.6+0443?âì^Ÿ¿ð¾À+³ý">5ÆÀ;]{ÜqÀ<g$€	@!Ã%	òó?ò«^Öw?âvÞñ'?ãÓÓÃt^@ÆQÒZ«@"6ÙÁ¿îè"1 ‹ü¿âݜ'éS¿ä5åàD"ð?â¼(+ì¿ØÖ'\ä¿àJÂ7óaAGNbcuNVSS J053847+044222?ï¼ÂՖä¢?{§³Ë7Ž?TÉ!+$Å'?P'6'À•?|lLïóɋ?yƒEGÇdº?ïVü€Ÿ?¦ÔQ8r[i?^蛓¦†Ù?mXph¢¦?"O–Ëpò«?¦[RÛöߑ?íäÒçæP#? '
,õŒ?z×Á2+t?zµneQ»?®WÙP€Ûd?Ÿ5D¦X?î(ç
{ú³?"îM_‹)4?Wê_aØ??S;¡¢Ä¾ö?¬²>e<?"Ééhïž?ï`ÜÝï'?–0"%8?sy"=v_?ˆ´7! Ùa?Ž<F¢é³ê?Žg—•'¶Â?îlß@0¶p?·üÁt¦†l?xI]ÓÛó?•Õ>òî•?¦(àEÝý?·z žàD?ìKL'm5Á?©¿"cG?'¤@n‰W?"IŒÇìA?»QݜA®?©A.Œ?ë›jGO'Ž?­`yV?aݼL¹¤v?fË
¥¬i®?ÁJßñ±wv?­O%E\ÝAGN4FGL J0538.8-4405?Ԇ—N:˃À?"á¬WâÀ6…C>C1®À:áUÁÓt‡@¹&>{@%ن³U?…/‹]ìšH?¯¿!M@$qJG
@"_ða俚£xHCÄ.¿ÝUý£z´¿âŠ¨ÀSÓ¿ás¤r:¯ÿ¿å~bÁ–7å¿æHdÞ&‹AGNBLL3FGL J0538.8-4405PKS 0537-441?ïÓË÷Ä?w
ÔWWw?I5"¦c]ý?Q›Ï#Ë(‹?róQ¾ˆM?sóÈ¢»=C?ïÀ×'»þ?"Ð2¾áU/?Q]jâ÷"z?iþ›mۂú?{=‡¤E?€âíxþi^?ïT´Óöå?"54NÃî?ytÆ>Pè7?††3q'µc?Žh(HΚ?Cø­oG2?ïø Ž§~?@%i¬ŠªS?'è¸ýç?K<	Uí?M+¤Óꇛ?>)l"=?à¥i(?z†z֞b?SçG$"M?Uå'‡d€?…¨ŠßRlj?xŠÆè¾76?ïmì:·r.?˜olm"5º?\N]Ùî?qŠh¾û;í?}'ËöÃS?–îåCÒm?ïQC°ó—+?"¦µQ%Y?xc¦žƒn?…gÛäöAï?}@uûŸ?ï4?ïï×2HE?UÅf»ó¤?3˜ŸiBÏ?ºS+o4§?^nbQh?U0ÉN[AGN4FGL J0539.0+1644?ÛZ­ÚˆÀ²ðZpŽÞÀ:?LÔÄèÓÀ<ƒræ§i@ À-+1\?üF€'q^è?ÇÄÚº÷f?Ð#nå;µ@`q$/Š1@Rëä?/@¿ïÿüñý?ïý~›;…¿ÜkÊSuÈÚ¿Å÷÷ÛÉ¿áL«tp–¿ìÓ51:4¯AGNbcu3FGL J0538.9+1646NVSS J053855+164612?îÎ"ÝH?Ÿ&ÿæX"Ò?`#_ôcìó?W§Ù‹<­²?¢ݪ09?žo·»32?íÄt1C?±)õ2ìR?^^
Ôo°s?oh¤%±ó?±eä2r'¤?°­§Ê]&?íÀ©Ù;ñ?›Ò[abŒ
?˜ά؇?}Œé[CŠ©?¯iP6àM?™T>ÁgÜ??n¢B?}Su'å¹?zÅ-a±!«?Zì1+p?£íæ\qÄ3?{mUªÈ?íAiVR>‰?¯_ÿ‡˜?uežÚg?kZo!¼Æ?´£®õ"5È?®§áYA|Ü?êRµ¾?ÃÓ+˜Ž?kø	iu«?z
o)°Š?ÇrÕf­o?Ãzîw†8-?ê¬þʺ'§?ª¬ê*ìíÈ?"æÁÐF3?Žš3î%)^?¯4ݦ\?¨…°¼G"Ô?ì±V4ó…?•eFÚµ?ŒˆÑ-+G²?w+²^­!›?¶åó(²úß?"áԓ7!LAGN4FGL J0539.6+1432¿ïûôGm°À!_ôºQ À93Ô¶¦ÛÀ;©žÙt{@ó+kh®À@}/Bãª_?¹LFT£w?Ågù¹iï@§î%âè˜@çZ™B?ïø¬N¨À¿Ýã܉Ù2¿ç1Ubˆ
{¿æ'òÁS¿î™i}Èâ¿á€‡—ůAGNFSRQ3FGL J0539.8+1434TXS 0536+145?îá9ã¯?¦½Ñ
¸Úk?}f«¹Œh+?'l8ÙT‹n?œ…m×bÁ°?¢á]&}8?ï…T#?¡a#}Õæ?J±­ ;Ê?Zft+µ‹I?›¨âo³? ûœ%6²?î'°Rîj?›5Åh¥b?";Ĝê–h?"aiÁ(™?¨v	¬Þ>?˜_B=ŽÂ*?ï·PVãH?`<lÌÞñ?T¢Öüâ¥?:ïb\7yç?/N{r?]íêݎ¥ó?í²4:€k?¶ÿàø+_?Sc
ĥ
?ªñ"Ù?¬´Ë6:GÑ?²æ*šG?í¿óegä?´<a¨Uc?^€üpÿž"?x»'¼½-?±Œürß)?³ë|QB?íRGËp¬?¤æyT×R?"'st\li?WÒ +–?²cæE-?£°#µ?ï(ìýçu?ã"L?pf¯5/U?\S"&kŽ?–È´r	ž?e•,&ÿAGN4FGL J0539.7-0521c¿á÷œ¶w¤À2_5ŸôýmÀ9ə~Á¦ÿÀ;T²ò03¤@¶FÉ)@0Þ@'—?ÑáõRýÔ?äŽàØóL@-d"¿G©?û½DC¦É¿â†¤^ïy ¿ÑYƒÿÔa¿çãW=SŒ¿îýÄupÅ¿ïþï~þbÇ?ïýß(ïãRAGNbcu3FGL J0539.2-0536TXS 0537-0524?áÞ	фº?È翹m?Ób ¸ö?Ç1"5Èþ{?ÁÛf´{.?¹¬—nœ?äï"?''?Ðfï¸Cå?Ð&»D}ø?Í`ù˜à??¸
ÃYw"?·÷2ÕÁó=?ánYR½Î=?²N"b†Ð?ÂeÐùFT?©F¸v(¦<?ÓðdÝáX[?°¢KÊ~ ?Æ©š‰"Ïì?£bV¥ƒ?ҘLÞ¼»?¬94ÃÅÖÓ?á	rî<¼§?°`CÌ?Ö=Tzr|?Æã­;.v­?Þþº@ê<?Ê?ú£Âñ?ÇMZ†‰F?ÁÑ÷Z;F?Õ9•ƒÆ"Å?Ðϒ¤ÝÅn?àÔo9Yú?Ò¨¯Ÿs?Â;k?Àªsw'(Ë?ÚLФXö?²Æ¥Rã¼M?Æa7^Ã?­*xyŽaW?ÚÃ+"¬š¨?³;Í8<
v?£¹XÓ`!Ä?‰réLLnJ?Öd¯ážYâ?¸ÆÜÏr?ã''MÓ?¸a1 Æe~MIXED4FGL J0539.9-2839?쫦ÕÑÀ;FE^®âÀ8ÜhìR¤À<:kHM@æo¨"µ@jnü7£?¤àš_]u?¼£çü(/@IŽ|/%‡@³puÞÔa¿ÒԽ렿æV¡ÍD¿é®/RÓâk¿êýDcÝ*¿éÒ%Âu:¿ïÿùëñAGNfsrq3FGL J0540.0-2837PKS 0537-286?ïù¯ës4?=äÙüÏEH?4Ê·ZµN?+^tO¢i?A‹ãµ'%?5=B—É?ïÉ5¯þú‹?€•;ÀüÜ?L/×½';?]àh6Õg?wß,ó>€¸?{Þ
Ò$ŸM?ïbÛGõô?‹Þê8õ‹?w£‰·˜@?'$'p=?‹ÇÜ5&@?†¶/…m5?ïáI"|+þ?OÛâª?\çvø^?D,ëV'\?`B°ÄÐtb?B–'Áïâf?ïñˋüot?RjB¸e"v?A'—UøcÊ?8êæè î¾?S§œHú½?NÄàØýÑ?ïi×"w_n?"H^9?gÓ×ÒÀ#î?}–­ú<?•Aqï™q?'-n` uB?ïY3ð>ä?'ô½p}/o?|-s8+t‰?'d•Z›õ?—i|¶ØñS?@N€"Ü?ï§a§K??p·HPsÊ?vªÉÆË¿{?fËWåör?u¤bwzÕ?bÈï¹´ÉAGN4FGL J0540.0+1209?àã']ëÀ#©QçS`ÐÀ:MY0ó½ÒÀ<ږ¹ëI@1tÅyÇA@b‹°¢Ê›?ÁÅ«âqz?¦í´£á8?ç*êßÝJÉ?ÿêEko׿ß;ž¼™#¿àÇ÷°¦%™¿è""j«o…¿åÂù¿ŸԿՏF¹!õ¿ì©«àn[AGNbcu3FGL J0540.0+1208NVSS J054005+120955?è{iÉ®p|?Ât½}_¸^?|J¢,9•µ?o®¡}8›ð?Í0É
OŸ?ÂYrfh®"?ë©qÍðØ?¹%
Þº¼Ó?j‹m4ª?p¿ñ‰{"?Àðb9/?¸Æ®—í?í©í=ñ??˜XL$ú=ý?€ùt;ŒV9?p›üÔá?°'g?—8ùN ?îH²k ?€Ã(*ñ¥?qÈÚ ²)?WS"?#??©;½øû¡?€ƒÉbÎÆ?䒠À÷£Ý?ÃÖ°Üqj?Œa¦Qý'?	‹ôYk?Õ÷±K€Ë±?Ù«]øið?æsº@œìú?È6µF¦á?s˜Goüú?|_ªn­Ïˆ?ÒÊ+Aø?ÈË`ę€?éež×éWê?¬f?þ\a·?'…3RŠ2ì?€ôœ¹^?ÈÞ4öy;?«ú·~¢k?ë
Î-䮅?œœ‡Ý?ˆ—˜[­°?vãUŸv¬Ê?Â?MÂDwm?œSª¶¤`AGN4FGL J0540.5+5823¿ïÿ䞝@,‡îõìÀ9·É°¸šÀ<1µ°P•D@ {Md·»?ÿ4ùÜÐP?° ÄÍ¿ƒäª
I…?×^ëîù@ê6êø²?ïªÏL¿µTÂ$'Q©¿æyWÊÆb¿Öt{/PP¿â*@Õ³P¿Á6"f\UkAGNbll3FGL J0540.4+5823GB6 J0540+5823?ï9ýÚ-Tï?"³-"²?]öٌŠÿ®?VJ·}=?–à×'C$?'ÚOh¢+?ïœ[£rû?ÏÒ뾸4?Væ
﹂3?bn^AÓ®Ä?†v£"îè?‹6ÒÛ÷»x?îÅ¥òԄ?"st«slÑ?sÃ*—ð'?€b.pCE?¡-?J»ž?">ãѲK?ïNrºîº?wg^˟˗?z%pã{?XA…lú?—n¨hå'Õ?u´Åã-E5?î\Å!ÿüq?£cƒtH+?l# ø
db?c5î#?¨q{Îož¥?¢Åe§!Ž?ïˆ|]@?› ¹_ó?i6‡xH?|tՒŠ°ï?›ÈÒÄ?˜ï`G(ã˜?í³¯IP£S?ž%vkí?tÚä¶M,w?x3Ëz
‰Ñ?±×j,!?]ßBëîî?íh±ÏñD{?"S7øyTÔ?"GÖ*6?xùèvÛY?¯ÑV8q-?'~œ-Á°ïAGN4FGL J0540.8-5415¿ÕZA"öÀ?ڄœ²RÎÀ9Ö­'¿À<0'5G	ª@P®äY†Y@×¢~D©}?·…ß'˜J?¶vÙ{0øÆ?ù¸ÞÙ>Ë@üwÒÊgÃ?éÕá[Ð
¿àÚçœr<¿éW°´hR¿é
Öøj
¿é–š«èP·¿Ó3«¾Š>ÞAGNfsrq3FGL J0540.5-5416PKS 0539-543?ïù&GŒo?:å÷I§ÿ?%ÎVLV\?RàŠ¦{ô?EóN-.?6‹_ïh?ïçŽ,†¤R?h&Ã~¾x«?2²ãt
]³?CóÃh?fvä?dú§±ml?ﮗ¼½¿?urº‡Ý?`Ã"ƒFÿ?f¾ ;#·~?€6I&0^¡?p¿'JÚ2S?ïîú%ÂԞ?@_íµJ©X?7~¦×é§?œ]•ýu›?\I"¾|s·?>ÑÂ;ž(<?ïóµØ>Ù?H—Úc>?1ë鍖??&‡ÛŠ,Çà?TìÇ<?Eíø³ŒX?ï¬@¸ç ?"þl/'ºŽ?Gýý¤F0?VÿL2©ç˜?ƒqúj&&?ƒ_
Gó±Ø?ïqò|šìf?ohŒ"?lŒ[Áeq9?o"=Y{?Œ`IÙÍB<?zÜÙÝÕ?ïÈàMKüò?d;Ú!?T€gäSÈÈ?A^‡F ?vo¿Pnt«?b(ÆÕµQMAGN4FGL J0541.1-4854¿Ó1Ō‰HÀ?[ÂôÀ;Jh˜À<»ú`ƒÎV@ I'ˆ°é?þláłU°?ʧ6eAÎ?±ç0Ñ.0j?æ£ø'Ä@Áp¾0a?ïà¿ÞQÚh¿ã8 7­ì7¿×@-…öú¿æûm"X9? ýÜåÑw¿éÝ}‰˜š–AGNbcu1RXS J054106.1-485408?ï˒ͯ©?p
Í+sù…?3Ÿí‹¬?&M¿VvO?xüõE$>ÿ?o]mÂóÔ|?ï°xÙ¹!þ?Z­âÝ"?SÑÇàPÍ?`kÃü¦O§?g£ÌÜf?y˜þ8í?ïER°" A?"<Éçlš?]—ÚzPþF?VBÝÇIè?•|,Kb~û?ƒè€
×±?ï³,maZ?cwtÖ"~?7H֏Zø?&ôEšBY?'zž,‡à?cP!|Ê%?yI~4?|íêÐ?FͦÏßn÷?:ŸkÅâú6?†lÇ2ì×Ó?|5ƒžžNÕ?ï<)b5:†?"hMf¸Ç?[Ñåˆ)¢?jWF}m?–½µey—Ì?"H5 a9?î'ZGõ1?"R®Ó±{4?g…¦/ÿ»?hÞÛtŒP?¥bZ€v?"E¨M3?îÿÜ%§¦Å?"êž°4Ë?LE­i?D›
TÉY?Ÿ"S
?Ô>?"ì¢\AGN4FGL J0541.4-7334¿Ó‡±w†ÊÀ>Þy!°À:Îނö À<qÏI~Ï@D>·Ë³È@o?¾[ðÂ?ÇÍ|µˆ7œ?´e8>ŠÕ?ìÌxžÍ5'@¹\Øs?îñÓ'é|¿æPµà!=g¿åt!N¿ã%€Uпæ¢'Õ¿ï÷z?·%AGNbcuPKS 0542-735?ïÁH¹ú"?i%{ÿC±I?Cn£Ç‰Ü?1QW'æ?|íΛC-?hOã›Üò	?ïŠ3Ÿ¨ì?ÃøT×?`ò¬þbD?`ˆì‹¥´?‰6m0wDš?ań9y3?ïz–,g<?tτ‡ð—?bMLVHK?W'Ô}>É?Œ×gZ`ú?r4L8–ã?ï³…Óé÷?qQ꫟s?pÐz±ÂõN?KG=ô}ô ?˜õp u,²?pËáÁVÇ?ïjßû ?¯æÚ¹xH?W…»ÕÔil?F²œË¶'É?'GHJ
î•?~wÛGP®ê?ÍÖÓ?–6³|`ý?pxHÃ=®ï?vÀ¬çTç?£Ê
æè÷?›$Qž!K|?ïH¢'ª
?' f0B^f?n‰ F>Ð6?a	×ù';?šE·ºÙêž?€‡J!
`‡?íIÂû#¨?ŒbŒ'&â?†YµŸ4î?kòw¹¿9?²æ±…¶Ÿ?1'®ño™AGN4FGL J0541.6-0541¿íÍò¨mÀ2üÞãOÆÀ9®Äjþ{œÀ;]±÷^pÏ@,¤ÅFƎ@ÙEnŸ?ȪÚ3½œ®?Æ6·L2º@	zÓõ@S¬–¡l¢?ïþVèD!˜¿à.ñàW™¿è:#aÔÜ¿êsp-…¿ïçæcvÇÝ¿íyº×AGNfsrq1FGL J0540.9-0547PKS 0539-057?îǘBà?òpû^¾N?ciä	"?_q^}K?¢Oê?w¯Ò?œÂ.8¼Í?íxмq?²°«ù«m¦?£°NmÊ~?§:"â±>?¤Â±Š¹óO?¥Âh™L?êuT¾\‡?§»mÍå…é?bErÃ?'…î…Èñ?Â~j>7HA?¥þš_ž=q?ᙃ«Šv«?§·Â¾Dãy?·îŸ"*U?•×Á9ÊÔ?ÖÑPÃD–f?©('¶5?ì'ë–]òF?²hžYƒ?ÉÝT`?{_ÊåDÔx?¼‡g¬¦U"?±¼Ç Yt?è¿dZƒÀP?Åâ2;ÞÊÉ?À:F¤ô?À¦¦–ñãL?¹Qá/?· `‹š£?ã¡ &"+Ò?³{;}J&Á?¯éb9AP?Š.:ҙ'?Ô¿†°€2?²dÑ|9*|?Í*ï0¾©?¤"uo=±"?Åå?—<¤?¯+Õeµü?ãBe^dËm?²ÞꎉMIXED4FGL J0542.4+3547c¿àµx{æ"@ÔÏr™À9{ÿL{ٕÀ;/(«ôž@ý~®Ü¡×@cwá¸í?É©½(?^?lj£Aãû@gÀôQv?ø?	ˆ??ïÿÝ/ñ_S¿½èplN²Á¿é}ž¼C¿çQ˜Wz:¿èªŒ€¬bÊ¿ïý¸È3
AGNbcuNVSS J054218+3541490?Ô€EŠ£²?Õìõ??Ž1?Ԇ?˜	T]<€–?å;§85?ì]è#Ñ}?à9üq8?Æú	#Ç"?´ìÏUûûˆ?©Sµ{éj?ÚPÔ¼.?Äýo¤J ?á÷-•u¯?°Õæh}Ž?«fL?g¬´?˜Ü&ãÂÓ?Ø¥K?°ú¤›\:´?Ú GðÑÜ#?¬žg¤H?»@˜Ìj&d?'Õ
Ê)?¦?ޏ'ÜšD?¯qO¬Té?Á½Üí´×k?¸G
þ0Í?"§¨t)§×?—¤šéʾ?êëKCó†?º!‡ñóÅ,?Í£Âû›Iû?ÄÁ`ÆFÿL?'nÍWÐæ&?Ãw¡J³é?ã4›ë$óø?Ê|©ÿm]ü?Öæ1o01?²Ò—gX¸?¶»U
F?¡^´ì0jV?â"E¥%¿?´ÄN™®!?Èú-ҏô?¦ñŒíI?Â\ü¬´?¥KƒZˆ¥?å*5k¥H,?²`Ä)ÔÔrMIXED4FGL J0542.8-3458?ÔâäசÌÀ<u?|ÌÀ;§W>«6zÀ<åÄ÷u³@ Ó,nÈà"?ý<ÙTšŒ?Ѷb'œOV?¶wÁ­‰æs?ènò&"©x?÷p'¢Ü8{?àÈ'Kžd¿ãÏi_?*¸¿·ýÌ^'Ýh¿àG>îRX'¿ÔÎÄɞ¿Ü œ'­ýAGNbcuPMN J0542-3500?ïĎ7:Ô½?sAu&‡?+ýÓËQïL?!M\

EY?|ØõÕÒ«n?rÃ͋â?HRÌx?ˆ= úñ?c½ÃïªY?iöa=Ù°?‰â|óÓ?"D˜—°E?ïg³ØV'?{-ªeÍAð?^ó%1(ö%?W>zD#1?'R£íÅ?yóQunŽ?îào$Œ7˜?yÇcÝo9M?ajnZgä?H'õ¤7¹? âfÔ)ËF?yuŠÎ'#[?ï€×Ü{?†Ö MLk?@5ºJ<?7
nBÜbÄ?ŽÉ•åñ;?…ºˆ¬«Qú?þ%Æt? ÓGCÄ!™?r'³ºÑ#?u«:¦'?¡ÔÌD˜‰š?øc…k|?îç^J'k?‰œÓ¼?eª™"ÞÈd?jfAwùq«? /qÂñôÓ?‡Ô3?ÝB?ì‰E§1»B?™Ž5Lÿà?qÚ	lT'ß?fG'Õm¿P?º˜2.ƒÿ‡?™Pßæ=AGN4FGL J0542.9-0913?ïäèuÛàwÀ3^rÚ/­À8Óp]`-gÀ;*[rÏ*@¸	FOÆ@×üMÃØ?´ìÈÀ£ž«?ÄyÔttF@¥!Whœ¢@ãðŠD?îÛD)$¼¿Üø,AQ"¿é¡Þ¹q¦¿æ# ÄS¿êÚ÷½'E¿ï´~!nÑAGNbcu3FGL J0542.5-0907cPMN J0542-0913?ïÔeLWhê?k¢O83?e˜E€Å'µ?aTKò‡?fmåÙ¶?[¥}"‰œ?ïhPgæ2?"5–D7ƒ?vµ/®¬Y?|ÂHO%2d?Š'N7¿/?I!w˜?í\ÿi¤€Ë?£Ù{¥Ë? ÐsßñxÆ?™‡û¢‡±?©_•'Vޓ?šËÜÙ;C?ëý	¯Åï¨?'\³~«©?jÈP]?zïžI³Ó"?¸½mÏk'?Ž=z	3?ï{Y­ùÖy?‡¿g±?|­±÷,öo?y…ŒZM?'Ò»Û‰?}í¬n?î/Á³¶r»?°~±à3ß?•ÿŒÉ½Ô?¨¯	4µ}÷?¢cÜj?£2kÉ7þ?ìv^<\Ž?©Ä³Â?¨m±(ßü?ž'íãPzt?²Í½4¬Ä"?¢Šã$ð(?åsªPdá?¦{Ë˗ƒð?¶ß‹Eô ?˜âeFs?ÎÁ':$"	?¤-L~âßAGN4FGL J0543.9-5531?í°ø;C*«À?z]9–úƒÀ8´ŸVqüÀ; L?b@êˆü¾W?ú'åÂg=?¦ –R?±Íߢú@ìÿdύq@)øH¦Œò?ïÍϖ«¨¿¿Í­$Ù¿ÙW97Y2¡¿Ôh>Ã4G°¿Ûï?='—t¿Ùâöúó¦«AGNbll3FGL J0543.9-55311RXS J054357.3-553206?ïòo)Dµ?Qsþ`ŠÝ©?.–±Ê»²…?(B¬Oì?WN×ftLZ?O|">¢Tå?ïۇpÑ,?r}DëÁ«n??nS|u?J•âz!­?pB¦ÔѺ.?p±øeú×1?ï‹ýçCh?ƒÊr«ÌR¦?`ß ZÇ*…?iE;:Âr?ˆÈž
*?'ocJµ(i?ïW`–L™?sD#µ0‹?Zß«™oÖé??ðç¬Má?"f°‡Ém?r¦Ôù•¥h?ïáXˆ_èü?fЀ6¢M¥?@ª•/ö"|?<ƒ8•Ô#?j|Ò?{¶?d"lÉr?ï—Æø™Ñš?ˆ:¥ÏO6‰?UŽ>ÖÅÀ?nåf(­c?‡\z%÷:©?…ç5Eìz:?ïr_x-½?‡MúFÉN?c:T'†?oŠðyx$?Ž¤SOëø"?…Ì'v©?îµW_YÏ!?Š"lñ èN?h^"•l;z?T±r'¥±?£$§ä'ã¸?‰úÞ±ecAGN4FGL J0545.0+0613c?¸âîë¦CÛÀ'qýiôÀ9ì0Ûj'À;¡[wN@ź+µe@ñèæ?ÎUlƒ‹æ(?âÕýÞâ@†I%ÿÃ@³ƒJLÕF?çÕ7Ÿ©~¿Êø›‡°c¿ê¤0ÌP¦¿ð?ð¿æbb™RLAGNbcuNVSS J054529+061955 ?ìîò*n,r?¸úÀb÷•$?›Þ3¸•?­=/A2?±áæÄ­Š?²¢‰E@?íã/Ïiˆ?·Ê^W2É?Œ_´i«I­?žU<	«s?ªµôN•?µzcãôŠ?æ…؋iM?±zצÌ[Y?½3å	ÚtU?¨.¾ÃM?ÇQª
â ?¬	P_ä£ ?íë3t÷xÈ?žDŠqÔÙ?näùËÿ¹†?o:RKh¶?¯^yv»l?2ÂC½â?éƒ^'ã?Ĉ %öoð?¯\üAoç
?±Óü¤:cQ?Âsuñr?À¥b&Þª?ë|hÜ7y?ÅÕ®eâ³?®Efu+°p?»ò¤•Ô›¬?¸)i~ö_€?¼¯C|¨?âÈ
Îæ?µÆ˜>pk?ÅUštó?°ô¥êû?Ñ=¢åjú?°{nêá?çyÊ£@¦'?ÀÄB‡?™"¸úŸþ?? !ÄÉ8¼·?Îæ^T…Nš?¾•`œDfAGN4FGL J0546.9-2206?ìg"þÀ7 E®_úÀ;~?SÒåìÀ<̍‰Àß@!
¯Û¥W¾?ý¥È–Ý&·?˸é?©"ô›ó»ú?⥡õ¿?ÿëWã俗…"úÙ®?ïùõß덂¿ç¿Àéz-¿Ö—
]¦ú*¿ã/5b7'£¿½ÿ¹3<îHAGNbll1RXS J054656.9-220500?ïè·+ZÌ?[X,}ë ?'ÈúÐ?ù¼ëÊý{?eÎø £ì?ZϞ$w?ï»ô;ÀdM?y¥ä~5å;?PÎFÎ1X?Yގê^Æ?}ÒPMUk?v '€}Œ?ï.Flÿe?w™ê¨z?Y5ËÀ'"³?AóZé¥1"?Œ´ø´v?vÅA™ý?ïTãÏG,?t Æbê?lH%U™¡?R"ª«¸÷?'Útrq O?sç͜éúÂ?ïÚ,yä%7?b~_QUOk?8Ü(9Ÿ?.cä>'x6?qa¥.öª?aá÷¹X?ïO_E­*½?'L«O/°J?aIyÎԋ?pøĜ܀?"êèôCò?ï7hž?ï5Oè"~?€Hœ£Äñ?`Xpž?N*â;¹n"?—U?×Ä=*?ŸÊ«qH?îf€›#?h(Œ¨.?€]Ú¥È?oùàÀ*?ªV­p?h¼1="AGN4FGL J0548.5-5218¿ãZèåÝÀ>‹¨çv°À;dÿÑÜ×À<àNú9¢@63Ÿi½3?þ^Õ®Þ]?ÓDE>Îqè?Ý\Šû>Ë@ØÌ<"Í@à\Õîßq¿ïÿ¾…{ª?ïâFj^?Çi^GG¿á'V½•!¿ë•ö¬š'^¿ïíFõ‡ÖùAGNbcuPMN J0548-5218?ïa3g='?´ÛSn·Ð?"è} 4ƒ?´û%Cß½?'ʨ¥9+¹?w(4ìä¡Ø?ïp=7Ì}¥?Šõ('n¢¸?ik{}ì–I?l³$9KH?•Ó#n"2?‡"—CMéŠ?îg³cš.?˜öó+ž;?ì@ÒÐi\?‹¾ä'øPð?¡´`^(n?"6€ƒX?îÚ	ûù­x?{ar–¨G?…A÷'%å?h¯Â•h?š÷ÿÙÔ?vZ8SˆZ?ïʃ­…E?®ºéÆ8Ñ0?Œ'3Çù@ƒ?®¶_øô?Ž»+BVšI?'hŒ9û?î^!Ÿ?«c%¡»j?"w߃µa?"ŸÙ.
?©(!D8ã?¦8zÕ:,í?í‡ô'7A$?¡‹‰€YÈ?˜"äFì¢?þ]#سq?«oE¸9ûv?œˆwËM!Å?í~ÝÆø«?"•Ö0À?':^#5Š?~³ŽW/¯?¯tô'J&þ?''†÷AGN4FGL J0549.0+3258c?á7Ý.V@Ä{'W]µÀ:e²ÑyøÀ<Ô€ö@ ύ3YÉ ?ÿ­*:f-\?ĚS¾C4?²þ½à ¿(?ïïãB/$†@‹99\˜?ìÏt…
?í÷y´!]?¨]‰a×Ð%¿ãµÁM<ɵ¿ßЍ]b²¿Þ•Á}ŽK2AGNbcuGB6 J0549+3258 ?í蠑@ÀÌ? ŽÏRms?iÌ@f˱²?Và%U¸5ì?¯Ù2èˆà§? Jšþw?ê.Ëx›?Áf~,^`f?ueWð"?~‰öÂù<'?Ç4X6‰?Àäå´Ìa?í×øá•9?•ÆŽýÛÎÍ?y%FE?jø‹	7ø?¯[ÕtÙIG?"ÎÃòބZ?íy"*Ç~Ú?ÿoë%4?ˆ	ƒy'0?oÖ`سŽü?±2®:"äI?ŒU²ˆ)¹ö?é­¼	lK"?´§I'<÷?…J"òŠ?xŸLàÓæ?ÇôfŠ´µ?´V4Ûx
?ã†<!ÄJó?ȯÎÄô'7?';ŠT‹'P?'|;P=N?Øa«iƒYð?Èàƒku?éÂë§ÙMd?©DæS¥|M?‹\¬{Ä®?{T°––F?Ç>†˜µîå?¨‡Ó}ÓÛÙ?ê5Γ¡]?£®2 ÅÕ?–! øMM?†^iûmà]?Äf!Žox?¢ŠÐ"µhAGN4FGL J0550.3-5733¿ÜV y®ºÀ>´üvÄÀ;‡‹z&À<§—…Ã#@@§c±«3@¸¤ÁëÈ;?Â{A–£E?}s±¸ç?»i"d O@3Yàqs?ï½|˜%¿Ý¤q"&À´¿ç>A¹Þ³¿äz/ ~û‰¿êBª¿±±=?ÛÒHÂf—dAGNfsrqPKS 0549-575?ïg³ k°?µA³æNè?TYÍiëW?`Û¦Xh§¬?'ÉšŒÇK?µÁa­Æ­?ﶠ>_[?yN"Å9—?PØ^´#™?R"åæ6[?€T5eØA?v†nxìkr?ï>Út']œ?Š¬¥§ÿ>ã?j"Ê	?ñ?sÚ˘?"àX$ACe?‡êk_È?ïºàc'†X?^@Ät›SÊ?P'Ûaš	»?1¹¹.)¸i?~orý²?][q€ÎÚ?ï	jʤ("?­#if óÖ?dÑÀÉ~¤¤?[¯qš›?œ8n¿Eõ?­ݽËQ?ï0‹ÒËX?¡}Ç&+?_
9¯½2&?iÏ$èXÂ?šIîFXÐ? ½Ã2ƒÛ£?þ=ÌÙ?'I%'H¸?r\Èf	l	?sÍYö§¢Ø?¢é7²k?'Zää+õ8?ï61?~å3
-?jM.¦˜oø?U;TßM†?š"
£ý?~©³XäüAGN4FGL J0550.5-3216?ל´è:ÎÀ:.—á2µ_À:EÂHåL À<eg?ª9û@ 2x'$"?þÔóý">6?¶™÷']ῚÎL‡JÀ ?äØ<l—ØÏ@–ß~*R¿ÁaL ?¿â™baÉô€¿ãžë}'ü¿ÃøÄwhÂ6¿åø£_–¦¿È¢›[e¬AGNbll3FGL J0550.6-3217PKS 0548-322?ïäû£G ?U'á–ÍÕ=?<'^e‰ØÔ?*¥¸ê\S?gtŸù?S·ßÝ¥'?ïÌIÔ¬·{?ty؝¶?à?EòvïK¤?O‰DùNçY?wÆà{·¦?qÆݔB/?ïz.¸WÓY?xþ,«‡|?aö£]É?V¿—GŒ?.Ôfº˜D?xÝCciH?ïWµ}>³ß?jcØÂyaÁ?hߑ¬'ƒ?Hgú…'¹k?'tfÏÚÙ?hœ—ãO‡à?ïȔÛûœ?j¼ˆoM?PFüQif
?@ƒÇŒ°?w¤@`4k?gqÁßb?ïa‡Ié`µ?ªuzyš€?XsjÌJȅ?c| "dwÝ?'Gàë#Ü?‹·œ<uÌí?ï­šœ<Ñ?"J',õðr?laƒ&][T?eÿ®…ë»?™~Jtw?'Yno˜?î; W×`?…£Aõ)—?€TyPç4À?hfΫ9©?¨0Ü.Ô#º?"7'ã4ŸoAGN4FGL J0550.9+2552c?àZ&|ä¿â"Ùîô?À9æã3@Ÿ-À;\€¸!D@q`-…Ÿ?þ£Ah€?ÔVK¼J?ä±il«$@'Á¯bY?÷îÿ&¼,¿ítD
õ?í®¡žJÙB¿ÞГ@d8¿äì;\Í`q¿ïüá1ޟ]?ïzô}jäÐAGNbcuNVSS J055119+254909(?ÀÒññ…¥?·"úáöA?¡Í? "
?²ÙB™ž_?ꮫߗTÆ?½½2ÿ?ÉOoEæ>?ÂrpN¶`>?½@"vsÌ?µ$Æ6?æÉg˜?ûZ£Sp"?ÔDÊ[ƒ?°³^í}?»CÀ½'›Ù?£(·û¡¤ë?âu"Ý-JÄ?²z8¼pD?ÖY刟:1?´B§Ë?¼ÙT²®"?¡Íóü,/
?á7â¸z
?¸aÚcÙÜ9?±1'5eAÂ?©¿ ÍçT?£"™\{ä¤?«ð'%7?졆#´ÔÍ?´Ê3ÌRí?³êÞSžu?±•¡.¼Á?½˜å¥È?º}ÓÀ[û(?é߂"žTX?¾jì̶@]?Ç#Š1P
?«tæ½Öé?¼>'ÇN?£vªR	É>?æ¶ZÖ¡s?±<Ær?Ç°Åã­­?²4ZX±´þ?¼³Ÿeq°?­3/lÕq?æ}Zšf"U?¼Ag\
O§OTHER4FGL J0551.0-1622?Á½ÊG<«À4ŽùÛ"ÐåÀ;jNÕP)
À=<±¥)@z8MNgl@‰üpy?Ôa):¶à&?ïü辚Úâ@n'"šV@Ÿêw­‹"¿ïè—8å?ïý2%9þ¿«s€]æï¿æIàô¡þ¿ì³·RDÌ¿ïÿæÀ
AGNbcuPMN J0550-1621?åiê†_ïÄ?Íæ×ÿŸ¡µ?ÒÈZ¦ƒ{º?ÍRñî´
?£'iTÁô?¡G÷ô?ë†6;Œ"D?ÁØåΕ=®?·¤ðªk†³?¾‰Œu®?¨Rºó<•`?¥P1iÜ?å˜uNiM?³?Èû'`?Êò‡W³×D?¯í)¢[w/?½Zí¦%?¦8ޑÿ{?ímUNC¸o?–Ç+J‹?±	n'‹¶¶?"D+2p±?Œ_7ØeZ˜?}ß·ëQ7Ï?âßX}ùÇ?ÏS<j5ö)?×'jrd¡j?ÎúµöÍ?¨Ï$Ž&_??¥ Q›]{ø?ç Þ×]ÁÊ?Î*†ãƆ?ǁ~œàm`?ÊøѲÔm?·ö	™Hö?µcN¹3ƒ^?âÖɜ°i.?´¦Ó‹½>ä?ѓç÷²?´tP›	Aƒ?Á}Õ½Pæ?ªx%cch?èx"\VÔ?²À»%€N6?È\äƒ3?°£rÐú?¥"å´Mš«?™ŒŠ•hAGN4FGL J0551.8-3517¿à~kÊö«:À:¿ÿ›V2<À;_ø[ÆÐÀ<®}1"Š@7ÐVD/Z@80êÄ?Éãã¿­€¿ªÕ!ș?àèøFΫ@û‰"Óê¿ÐÊaÛ<Q¿èsáÿcøο蘰C)J¿Ò·ÇíiûF¿áß& {±¿ïÿž´JAGNbcuPMN J0551-3515?ïìK¦U??S–'G'Á?8IxkÌ?'nÒ¶½·?`±!ênDí?R3¹T?ᅧ»@™‰?|5Ô×
?LJ:"zÚî?TM=tyk?|±Züàñ´?xç)g}ø´?ïv-¾Õl?u'$"=—³?`Õ*b(çô?Yû"à$¤l?Ž?E·°‹?s®6Žù?ïÃQçÌq?_ßԕ.Ø?AՁUÑ¢?*b†Ì`È?|ä?^¡!6R?Ç?ïËm'2O¼?rN™åʗº?J%gr9??tïW®$Ã?w">à^?q~Ŏm?ïAu8Cò?š
ºcOæ?[º ¡ÌŸ?iÄB÷¸¿?–#ÐL…ªÿ?˜"´¯)
×?ï¥ô?ƒ C™•7i?i÷&ŽÉTÈ?d²m[¾8Ö?šìz¯L
?''ʃôý%?ï7K¦
…?htWZ¢?[ZWWj?J£ù=ƒ~Ä?—lím?~¼(ðþ#AGN4FGL J0552.4+3755¿ïHsò@#Ü@G¹EÅÀ9£4EHßÀ;º]éÀ"š@n¬`@¡59°€?Á—O Ò?Á2ZR½?üzžF§">?ÿÿa¨â¿Ðqm*¥Æ¿à)û|ÀÙ¿è¤@¼ˆ±ë¿åPŸ?J螱Áƒ˜{¿çWÿñ<nAGNbcuB3 0548+378B?êYì)é?²HF{ˆŽ9?–…Æ>mlù?ß›hÔ?ÃǗ#º¡?±²'ž«Q?äÀ­+
´~?ÛܡÎhÑ?¥›T'Ì?žÝƒ¿—Î÷?ÓÚÒI
?ÁÊj¹/?é‡ñ/ÏóÀ?ª™5ůƒ-?¡ Ždä–?'ÓEÍX}?ب,Y?§dÊ—v´?êUy6Ö4?–¹b²ˆÆ?£Ý±#2õ?}ñËúԋ?À"=Ð×.·?"o5'ñø?䟥Ì»·?¾%ùŽÌ·?³M?+—'?©·· 5§?Ñÿ!ý¢®?»+[ð¹•?،q$QæI?ÇŁ‡‡¦Û?³|`Lì£Ê?±HI‡e#?áJ;dû'?Æl)§vڅ?â÷ÙØùÖÆ?³¯Îxï6?³ŽW‰µü? Ž]mÐZ?Õ,¶‰`Þ´?±žø$Õ§†?ã•åEGg?©È¡×Çæ?¸Ré&·´?•Þäô®5?ÒÒ »ÏÆ?§yáAž¼áMIXED4FGL J0552.8+0313¿áÖÈõ¸åuÀ&ñÖ1riÀ9Øe8hýÀ;eQ‡²‰@q¡L–[¢@Fü"û­‹?Ç´°¶Áš?ÑàZ]āO@
ûÅ<@ÿ7VÙUœ¿×í\¤Æž_¿ß&H>2?ÿäÛâ…ï¿èòÁˆËëü¿å«hÎör¹¿ïþ3AGNbcuPKS 0550+032?ï@Ü>.äÅ?"lBqµ<?jwap;\?eI¢mv"¹?"•ŒóQÚ?'òiL«E?ïяK¯M?¡<#UqUì?v֔,åi»?€ÎwÈ¿œ?–ð)•œñ?ž­^¶÷?éé‡PŸ]\?¬åM²@Ü?˜É\_9fø?`Ý×ø?Å@·2å81?«ñãqNØÈ?ënÈPú«?–'Xó&ÌÊ?'³Ç¸‹?fŠåÀœdf?Á¢N°"ƒ?•Ý5&‡¼?îG°"[<?©zN›?sÈyLcX/?p¥>'ý5?©çŸùên?¨¦ý—[V?휻Zµ?¶x&÷ùfØ?•âH¤dï?ª">¨¹‰?«C&Qj¯5?¯Š´©‰^‹?æ²@x¯Øå?²\É3x?Ÿ9p'U?"3ë6f»Ã?Ъ‹}æÏq?±Ø#ÐN=y?ãCš´vÀ?­ð*XšÖ?›10@èè?†­n³Èœ?Øõ¶·ó?­¶£‡Ýn+AGN4FGL J0553.5-2034?ìÍ¿ª5¯KÀ5ž YžØÀ9Ýu&Ê;À<­ê‰v6@~¸w«?ü9 4¾M®?·
´ÉuÕ?Ã׎\Nµp@ÿW}•@¼E˜•?ïüÀO(\¿Úx6<Òï&¿Ñ°'#Ùy¿ÝóÎCoks¿áè–!?é¿å[Û]‰HAGNbll3FGL J0553.5-2036NVSS J055333-203417?ï9µ-s×?´ëQkYI°?™‰Eyáâ@?´ñðóöò?j|Т߱?a‡ÀÕz÷¿?ï±ÅՌ¹â?€é\/—Ñz?\¥ôjNi!?düøl˜o?ó˜2ý0?|`1sãx?ïxþñ"‰‰?'˜Á±ÖqO?x7¢Pé}?|ãòú"6\?…¤rq©¾ê?uÍþz²x?îqÎX¥?{€A‹E?}jFØôþ»?YÆ@çí4?¥5Öï™-?xó3w©jT?ï'"÷ 2z?¥`z¸.ºf?"yº^¾¯Ü?¥&TZM½ô?~VšàþGm?tûû…Ö=?îå*Öå¡Ò? ú°kjO?|OzԖ÷|?M¤éýáÍ?œFÆk'RÜ?™?´fr§r?îÑX(ÏÆÁ?"¾¾ÖºÃR?Ž‹D¹Ð?ŠÁ¤ êS?–X'`¡?‹¥Še4'?ìiH›¥7ˆ?—£õë.V?'ÌÈý?s'dÀðZÑ?¹a¡'1£?–(¶yñ€AGN4FGL J0554.3-1009c¿ß!q¦3[À1<yÄ<hÀ9ÖÁ['—À;¢˜¢ô@>ñŒõœ@W'"¬Ó2?Ì°rùòŸÅ?Òc¿m@ë_ïIÏ@☡!"e?ïû%|'¿ÞôÔRÓ«¿ç¸}õÏ$–¿í—'"Yœ)¿âùƒ¿g´o¿ïü`8NûçAGNbcuPMN J0555-1002!?í°é=W
?¾¢ª±¼H?oŽ–*7h?e)绚†?±ƒXµ?¾àwÆØc?ïcžŠð	?™¦£y^"?'DE?Rbè?ˆÄê-ÅZõ?"±i¨¹y?"r¥FÈ|¶?ê(ÝÚ;JY?©—•z©~?£½AÆGBL?"ßðS¬Ô?Âm8%Š?¦O½Ö°hx?êöiíj¸A?"쮟?'Q²õ¾¼?s""‡
š?ÁÜ7µ	Gã?›ÚkÙ³^>?êä«À…
=?Ã?šæ†îW?ƒ3£‡5iE?fÂÍ®"?Ã:ÅFú?¾˵Ôt?í)ÀnMC2?²Õ6§×«ë?¢`ø삣?©e0îJÐþ?«ä%®æ2?¦ƒ7Bçz0?åY'f»åŽ?±5p2­K?²aBb_¢? /¶û½?дºá©}?°C\‰ä\ñ?å"†(~µ?°mtÚȘ? 7ÇüR2?ˆZšÙŸ=ÿ?Ó³úïܯ?°(ʇIÌAGN4FGL J0555.1+0304¿ë
ÇÇæoFÀ&¬ÿ§ëlÀ9•'ußÀ;;\ºëù¹@"©	#?J@X$¹ó¬5?ÒXDЩ*?݀£(Ž"ƒ@kE®_ú<@Üƒ#5?ï½<Á§TÿÆ?¹éÆ,Ë¿êz73rô¿êm3t¡'Œ¿êõÀv}4ß¿Ò¶žb+CPAGNbcuGB6 J0555+0304?îÛQô®,?¢‹®À	b?yóí^ýæD?}!\Ý­Åø?žÆªP3? ßùë·ö0?ê*»kŒ§)?À´ÏÀr "?ªMSæt"C?®å›µ?ÀÁ½WÂgL?»^¶%Éò?çTö¹3?°EkŽiEÜ?«ÐÀgϋ?›|eÝþ™?Ë·õý¹²?®.Çhÿ?ãòD‰­ú`?¥¥[£ý'4?¶ô+æ;£?'®îv‡õ?Ò^l(ê|X?¤¡f
®¬<?ë *Ô¿,?¾¤Ìþuç8?žîç;ÔeŸ?ªñ^¥Èi?¿BõP­;?ºMúV?I?ãYë"Ì?Ë#K»{?Æ/¾5/b?Ń¿£Õ˜ß?͓'•œ½n?ÄßŖUJ?âéeÉ?´9öø*¯½?´££«Ö?¢ gXȧ?Õ)ùݕá˜?²ájÑ®›?НQ)hY0?©4ÙÑm‹?ȉ8߀¿¿?­M}Êü«?á	3k£x?²­ü\ÝP©MIXED4FGL J0555.6+3947¿Ü†_£@&7yéÐêÀ8ÃÑv¹À;™Ø)!az@—v³·X@-µ@å£?¯ó–Kwx?Êe*&D7g@Á+àŠð@$5f¿&Ç¿ÛMÓÈi½¿ã½R ^DY¿ê¨ðN²¿ë-€@Ø¿î9Ìzd¿ïÿþó…õAGNfsrqB2 0552+39A?ïLoe@V?ˆ»&¬ô?ˆ‹ß9~?ì.[s?"XG‰h^b?w4¼í~¥?ï=´ÉÿF? «ß…JÒî?kqY¾UØ?w£ÑéZ¹Â?™ªLa…?Ÿò…'±+Ï?î_7
zs?› Rl¿Ö?•p™g'í?'s9³}›?ž¨"þ]ç²?"%ÅýɃ?ïpÒH•M¸?n{å½PÜ?x°…³º¥?]z@]ֆ?‡s+Njú¨?eµ"º#²?îù€sûâ?'·k\%#?ŠåÚÞÚ.?ƒDxѵ+Q?"]mµ?ŠcG«˜Ó)?íÃìV*4?´2îòœ?…è@hkh?£ªóv>Qž?®G* ãí?±—$'IK?íïÆ"ôô?¡@ÊÍ"šû?œ?Á'9à?–=ncä?¢ã½VǓÑ?˜'å÷êR‡?î8kËø]í?…øDML?–Øã\¿?ú†"'?¡lVˀÖÜ?†±¥W|Ž}AGN4FGL J0556.2-4352?åƒPàuÔ¡À;ö:\`‰À:&þìɹÀ<G|¾—ä@Á8jª™?ýª½þÓ°?¹œµØ¿tJ?ÄZã»Ñ§Ó@	®¢?Zˆã@	茿ð?ð¿ÑÄLá<P¿áânÁŒ¿ã©LŒ ¿è"¤o¶AGNbll3FGL J0556.0-4353SUMSS J055618-435146?ïø‹ýy½Ü?AU¯Jt?7IGgò?0Þñ˜ë?BNå¼ÏM?9Ž{Y×b;?ïۜ¹½.'?rÌlŽjg?ABò…q¦O?KùºÅ??p	D箂?pz`V÷ox?ïa*"ì?kîMñD?}¶PÒ?‡>áÝÃ#³?ˆÚVëL©L?…¾{‰	êÀ?崙é`×?`DUSF_?[¯u…\…›?A7—1‡Ê ?'Ä«Ú#£y?]C—PáfY?ïó8¦‡
B?P
Ö_?JÙkÞ0m/?@ã¡g?)ÿ?HCù5×Äu?F§ÁAŠ7?ï›Ûé¨Ù0?‡>üN¡vþ?S'û˜¤À?cž'12€o?†–Æ(ägÙ?…ˆ&nmŠ·?ïH4çÌ?ŠìVQ¤?|o'Žš.?'Úã88žŠ?Æm-»Ò?"x‹ä¥á?ïN Aiõ?xó%-	n+?h–§ü¶ø?X~wèà?")"윩w?vª,£õAGN4FGL J0557.3-0615?Öтéÿ¹À-ºIÂÁ±À:''¡WÓüÀ<*ý"û|ä@!7œÏY?ÿ—{ž?ÂàU*S懿t¼™4*:L?©¦^ÄԎ?ÿPûB÷?Þ­¥,tÓ¿«ƒÕü»Ú¿èí±´B'L¿Öð½!´Õ¿á,ï¢9Ñ2?²¼ŽŽ#AGNbcu1RXS J055717.0-061705?»¥ç?"c"?Ú©?N*8‡Eiµ?Bˆz†TÄ?ŠsՑvÈO?ƒ­RX?ï¡Áº[AU?†t
'v?W«P.O
?^¦æ§2?"š'v ­?"Ê!%?ï8é~ð\/?"á©Ï,?e¹ÂßN?Wä‹àgl?–Bíüa)?ƒ:(̦,?în—"¸Ù?"ÕÙk½t?u±Q«ø £?UüRh?¬RìN+ãÝ?"¹âJžšñ?ï+Ù^oeØ?"ßØ7ýù?_VšÔ÷¥~?_b×Py!?˜j|Ü°¬?"jÔ½º"Ã?îð¸Ý+¿¡?ªÁí©Cä9?n5¿‡J?zP³UE¯?ž(}¤Oèç?ª²ŽÚ2?î-_QQà?™jÁz°·?súÿ?±µá?o4ù·…*?ª¯š#6£Ç?˜.
þgÙ?êB	\Ë%?Ÿ¼>]~xe?ÓÛB×{?yí0}ؑ?Ŝۺȶ? ü–#¶AGN4FGL J0557.6-0721?ï¦KXÃæÀ. ù	kºÀ:ÔdÓ¿/UÀ<@Ñ0ߛÜ@!GÝcp?ÿ¢ºtÛt/?Èêo_‰Rz?Ê¥Þ©÷"?ÉU·­¢@ÂÌå¤?î¥ÉB©É¿Æ3IÃîVà¿ì"֎ín-?¦ùQÁ¿ßË¿ñò÷¿Í9б3AGNbcu3FGL J0557.7-0720PMN J0557-0719?ï¨+ÖÀI?–Ý4©ÿ?7,TGížs?1Sš™?ø?…;ÙqŒ9~?–Њqˆƒ?ïÜØÅBX¯?sÇ/ãH=t?4ôœëؔ?@Ü»}9ø?pDSŽÁÓ
?rºÍ€¯Èo?î±6Xׇ'?˜­= ÂÁ?aFñ'¶W‰?g=ºòl?£Ø+aÃïw?˜L6¿x´?ï"ø¶‡?n%ö3Î?Jï¬QAÖp?4³¾Û]äV?‰S4®>?m ""åb?¬®?ôÕÅèÙ¨?D	±5=ã´?;_Ñ8"?Ž—`ÇO'6?È]LŸ?ïœÄg+:õ?Ég¶ŸC:?LÝÔï©K?f8»ºÙ×?‡h]}ý?éZø?í½
GøMj?¡ûZwò_?dÌØC­?iú	Th;A?±q.ÿ7|E? Ô
®¯«T?î©iS+?Œào‰(Fì?hÉð	ý?_ºÙ7ò¾,?£â‡ºýu?Œ\e³BuAGN4FGL J0558.0-3837?ïf™UbCRÀ:mYėtÀ9¢&¶ÁÉÀ<.‡'§
ö@ʹø´²$?ýnz[æ±?³Ò<^'A?¬Ü	֘}?ù&رÝ]@4hwä?íCy1DEª¿â$;H«j|¿Ü»µƒ+ß¿ÛÕгÚ
¿Ú/¡ãêöƒ¿â¤®ÀÈ1²AGNbll3FGL J0558.1-3838EXO 0556.4-3838?ïß,Œê£f?]	y ‡Ï?:™W'£·C?(IÇB˜?m€HCtv°?[Y'^º#?ïωÊ2'x?r¾öSžL?F§¤'íèn?MÚÝè{?uf&q¤.?pGÐ^\ï?ïnó"¶Lr?x¾®ßûu{?cCŸ¿[ö¥?^Ýñ"Òā?r6èÅ1ë?v=ùŸc"?ï5ˆÈýê?n¶fD@Î?nëB¶`?L´QâòÅ	?•q~'c;Ð?l+B\ɕ?ï³JŒ¸'	?qäý=S'¿?SLI*Rþ?E'+D‰T?€ÃÙ³¸ó2?p¦\üªg÷?ïr‡°$©?‹U' kµz?Wå=kwE§?a
èsåâ?0ÊKˆ×?‰>Oç‹úQ?îΫU?Œ]c<Î-?qí¥O§R€?gEm{B? áࡔ/?Š0Å؂[¼?î ÞûV+?‡û3HŸ?04¬T9B?fÖU°N#?ªQäâã҇?…¼ ì¯wDAGN4FGL J0558.1-2859¿âŒ}|W"À7™0ߛÜjÀ:Ñ]ÓÀ<šz¦]Í@Œ›Ág
@æÜB‹–?˒ºNðÔ?Æp˄£=\?ø™åi{Ĝ@Ç9©Ml?ïü›ÇqC9¿ã¥ÞPݾ¿æ4Š¡.8x¿åÖÇAÈwS¿ïüõ$®5¿ïف±E‡ÊAGNbcuTXS 0556-289?ï+vÈ«¢?°ªZÊ
'?"RÝ6Œù?°?Bÿyµ]?€OhËw?uïÔ,J·?ïb³ÿKz?†@døfÔV?i›ž=ڌl?l=ŽÅ™ìj?‰ÀkqfjZ?'¤þÁ­Z?ïWò\uÄ?€é§ï2Ö?pˆîÊ?h§²³/ež?ß±·å¸k?{þ-à‹
?ïB°ÓW.?mRX÷Úe?}dµšTÍ0?ZÂUU?P¸<7Œá?fp¶÷¥tã?ïsæ›?«lwän?"eù£²?«OɽX#?'Þ¢£‡?‡ çvDå?PÅ.7?œÁȇ¤ÁÄ?ybž27?~"ñ‰4>?¢xø½«¦?™Q–Š@lI?îǶ9&V?Ž\ª˜h?€Û2åá=ï?}Œèø0h?ž›ŸnŸäÅ?‰ëWØM@?î¼ "ÅL?Šó±È6?'ÃÆ1àÊ?v–©%?§HTšºÙ?…`~rgJAGN4FGL J0558.8-7459¿ï\nW˜åŒÀ=†r!…‹ÆÀ9҈u"ç[À<U¼ö•óó@ÚJŒÁo?ÿ¦>{f?µì>A¯!ì?±›!ô›?ûHÆÆ#@ê¬0Êù?‡'ÑTW+¿ãf$!Gx¿áÓ/M= ¿Ü+%Â1h¿âG¦Ý¤áK¿åW¥£"ŸAGNbll3FGL J0558.6-7459PKS 0600-749?ïê:H¦7?P¼'-p–?8Tƒõ•J?&›KXb̲?b»6ú¡r?N8ô«åò2?ïÆᓃU
?'¿¦)¼?D÷‡Ú'?J͚$	â(?yðEZL±š?'$øŠéô?﷈ÑjI?j¸«Ém)ù?Sr™Ë¦°¦?;N¶!éU?_
³Ãx?iëÊð§é?ïn	¢¸sœ?föÿï¤e?f›¡kÞ?D:ít‰«?Žü0´%?eZ‰±j«Ð?ïÑH%Í]Û?bçQžµ?Nˆ3]‰×?<§½î¬
?sŠæ•ü!=?`Å4<ɐ'?ïI[£6GÝ?–¯'P•?Z‹C—é?dé¢?•+²è€Ü?•*q
vo¥?ïveÌHÕ?~N¢s‰š?cVsz±,?c}Ÿ®'»q?©‰«ÙÅÖ?yØÍk9Q?î{c‰Î[©?†mNò]S?|‹Mœï?bF'|o?¤¸]ÃÄTG?"b\ûˆhñAGN4FGL J0559.6+3044¿ã™3·ñž@EF%~>ÊÀ:Òn`/ë€À<Gfȋõl@"iôÄb›?ö¯•Ôèû?ÐWN»¤ÜC?Ú¾•Û}À@
¯H<¯³·@0&Ø1¿ïÿ£ž\w¿ïºÔaì""?ïþØ
b?åƒ)ë‹Ôµ¿Ü=½zÊ¿Ûö]"ÛšAGNbcu3FGL J0559.8+304287GB 055627.1+304251?éY"ÇUr+?Ám×½ýb?‹˜<û•‰?Ž´,"ôÉ?Èà)'W»?Á7Cmèæ´?çÖ4d¶ñ?Å)Ãh#1?‰{9QóLD?™'B¿ ?ÏzØt†÷?ÄœÂÕ
t?èÿÒuÙ ?±»ÊT¤&x?s"+…?""ˆzö?ÈRSX†m²?°H%R‡ÒÁ?êÿXb—¤Í?«í:÷ú?wm3Mù÷Â?lãÒßr?ÃG4Û1?ªñÃX-3W?ãÅÒvt?ɲÞRõà?¢÷ZÏ‰?²V¼¹:f?חEˆíœH?É ;x•×²?àHD¿o
¡?̜l)@b"?•Äš¥èo?¢>L|;'?Þš7	'·?ËÜÜ]þ'?ãöG€¦?¸†1šZHq?¥suGɦ?˜ñv ?Õq/Þ?·k­Ú
¦?å.+ŒuÅ?½±õ<úԔ?Žh/AµM?'M‡i¸¢Á?Ôðb¿¤Œ?¾Ž€)
ÈôAGN4FGL J0559.9+6409?ØìøÛc
@2èß?–À:þ¿yýòàÀ<´ZÐ0.œ@f™<ÒnL@¸<½°Ÿ?Ä8âʐž?¢Û=º?á°ê7.j@ž ÀêÁT?ïlËÀ]RÁ?£î˜àJd¿éól|*¿Î7UAPu¿ÝA¡
&¿ç¬?8¥
AGNbcuGB6 J0559+6409?ï¬ssj/õ? Ý;v½@?n-3"F? ÜˆLWV?z¯º«'¯ž?mrý>'ښ?ï±RVu=Ö?}å'7Bëò?U6ʞzÑ?YÆú8¼A?¦›FUB?{7ÏO‹?ïkC^¾@1?}î•Sµ?f³#	Ũ£?g3f PÇ?'_žÔŸˆ?xtu<~öª?ï'¹#ð?fpô$Ч÷?pþD³ ^?Q²"ΠZS?‡>Óª€i?cBo*%?ÄZ¿?ŠDÂrÅá?`C;&x?dûúÆ/þ¹?…þ**'?{2ýÞa¿?ï:R;-Ÿî?',:JȈí?eùùtV?p(ÝÏ|?–"ÔY–Ç?@fÜß½¶?îöÈ@Ëø?ˆœnŽ'¥?qSPç#'8?pF7Ñ?œÒ#¨ð‡d?…
¡áä!'?îÛ‰ t¢?…cB'wS?‰)èBm‰?sŸJÐ:Ä?¡—ÍT›³†?'ìxàдAGN4FGL J0600.3+1244?âã½&ü™Àú¼þ"°À:$™Õ(»áÀ<` SÇþ@#^ÎÚîùr?ø4þ"ÅõB?Á*h‰VUw?ń8Hñ¶f@vQElñ›@–A¬rº2¿ïÿ='—t{¿ï=ÙìD?ïÿtµÍ­?Í'"™2§¿Çh—Ð¹¿ÞqG ¨"AGNbcuNVSS J060015+124344?êTêTOÁ?ÀaOÕo!?~*Í.T¥Á?x
è&D>?ž1î(€ì?À7¢Ì¦¿Ð?è^
üþÄ?Ããú›'D?p·°)Ù»C?xïlôoßÿ?ÎZLX?à¨{"¤ß?êOGßÎÃX?ªé9_TI?®ð¶Å§?w×·?Ôw­?ÅÅoÒ1 ð?ª•;†«å¨?ëQ~'š6?¢‰4'E÷¸?sY;h¸d?c¯Ú#Ž,?Â÷ð/0!ä?¢f]9
Š$?åx.ÖéB?Æl}Gºð?'æÜ_ÀC¢?ˆ¨n¿Ùt?ÓñcÝ"b?Æ5z‹2	?à‡rX?»?Éþšdŧj?vt/î€^ß?‡Wâ¡W4?߅ [MÀ?ÉÃ{Ë?å²
ðQ•?²®cw–	?'Jü>ÅÝ?ˆxuÁÿèy?Ów^Ë]¸?²]3—î/?äÙ-úþÓ?¶9´¯©ë?ˆ9]¥¿Æ?ˆ<åg#†?ՋÙfh?¶K•,`AGN4FGL J0600.6-3939?àe'潩À:6¦ڜ™À9Çü6FãêÀ<"š3Œÿ@»3j:±W@nu5¬?»S9¸ÞXe?ÉJ®yûn¡@'ÌÛæED@w‰µËÔT¿±gû;õún¿æJ	¾Å£
¿ë«ð«Ï&¿ëژÒÊ<пí¤Qƒ€R¡¿ïû´áô|>AGNfsrq3FGL J0600.9-3943PKS 0558-396?îÇ:›?¹ÒßÀ/?=j'Ô¬?ŽlÇ6\sÎ?˜z9qÊ?¹­Ñˆ>?í5 b²8?³X8Ìg?¥*L(Ô]Û?¨ÃT0·`ˆ?§ƒÑӔ3¡?¢dÞH'?ëzÌLÒÊ?§ßÉÀ—?°Òÿy+ìÁ?¡N6ÁHZ?³Vž!‡œé?Ÿ%ӏŽÇ¼?î8Ç^pE/?†¦½ïdQc?œÛPÜW?€µ$Föo?œÃPÎÙÕ?yÌɏ³L?ìî
²£´X?±"‹<Ó}¾?«áZ¤@…?¦aoÇé,?¥=Ê/Ìfï?£ñU)h‰J?é‹~Tw?ÅÓћ5?º,"Ý
Ñ?¿ÝÓÎQdÕ?½,z¿0Nt?´ÓLø ?çäêËenš?±ö"Ÿí?¿%æ!:@?¬h‡îjd?ÀåAáiö?¦îþ˜$c2?ëa7I垢?£»#*r1…?³ègù\¤{? ¨œí'1y?±
ݶ,‹õ?"^tã(o:AGN4FGL J0601.0+3838¿íՙ̼@›%,à2ÛÀ9{ôörÀ;ýxM·‡@ 1ÊRt?ÿHécˆÖ?³«½ž¹þ?°ўî˜$?úkIÅEïÎ@¯–×óF‰?ïð'Þh¤¿ÖÊ'¿âµŸSí½Þ¿×l=Æþ¿æ·E¡ŸÍe¿ÉJ›Ú'†{AGNbll3FGL J0601.0+3837B2 0557+38?ëhpPcßg?ÁC><Ài?v×]r–W?oP$ÙÉÍx?Á§ƒÒ‡÷±?Á<où?å¾ì{ê:?ÄAtA? Ö¾a¶?¡ù«;?ҁMîö?Âz›XÜ?í]w­$€?œš\—m‹?"µ\!µ?|§,`/?² ¿Ò¹,?™´ÕׄÙ?ë©Éí@Ø?'¤9\wb(?£ÍZÒ]È?\åè¶e?¸Ë–Yë{?À*\\è²?çõÙF¾çm?»)O«J,Z?ë2ÊtÜ5?}©dwTÉ|?ÎI繦ï?»çC4vï?ڡݯañ¦?Ç
G¦²±Ä?¢ºã…êÈÞ?¨$¯ûše}?áƒbïþ?ÆFvz
jÕ?ê»fa͔?§Žf±1?"ÞåÂÖÊ?†­Jֆí—?Å5°C²»?¦%_©Ÿ?åÝ$—JE/?§}ÌÃoÜ?·CÉ4e-?–;fB1c?Ìé‰Èmº?¤&S"àNMIXED4FGL J0601.1-7035¿ÃhɁ)¥À=¡g‡Î•ûÀ8¹£¥Œ#À;è×Òª\@ñe¸°–@ƒ‡Ä"ÿ¯?£·¦J*ø?½Ò/ãšj@Fº z^k@pM6>«a¿ºŸ»Ç–×ó¿à*Iëœø¿æÖ`)5ƒp¿åЬÀ½ÊÑ¿è·âŸÇÛ÷¿ìT*Ÿ:î>AGNfsrq3FGL J0601.2-7036PKS 0601-70?ïIo«GÓ?¸;¼÷E0?îèÇñ?¸=™À¨H«?{jé¹ß¸¡?Â.¦ð?ïäÙó@?iCŸOX³@?9)§ßƒk¶?QÔU`š?hKÆY@?fbaäÖj?ﴓQù>g?}äb\?î?aU·±ûlË?mŸª,ŸR?}{,rÙú?y$"h¥?ïô'•û:°?8ǧɺÕÐ?0òeâ"]O?&ö¶bn?R :QóXK?5lÉt¦Yä?ï!k~Âíj?¥—…','#?€sć&Ïö?£¤>Ô ,?"˜­éæ@Å?'6Ö÷÷]?ïµ9Ê?îq?Õ*ç!É<?J÷¶¯Mæ¶?a¨s¥z_?ô½`W?€Ø…kÒõz?ïœì¯b¦
?'^¿±æ×?et"üŒ%?oš-J^p•?ƒg˝ ,ˆ?€u¥€ýöK?ïâ8ÓÂ?Y]ã8ˆ­o?FAÜÿ—õ?5Ã伤ˆ­?hSùTÔ¾j?VªÎhäá
AGN4FGL J0601.3-7238?éázÍëI©À=‡·Ïå†À:øz§fÀ<£ñà'Œ7@\\sôC‰@âÃäƾ–?Ä wÚ,0à?§—j•J?åü~ìC@~q'´¿ë[þ*?ïô¤'*è¿ä?ʅʯ¼¿æ«QAç*¿Üá-â'Z0¿Î±k

pAGNbllPMN J0601-7238?ïátoú ?]õû¤7?8] áx?+IBÙÉ?kìè'Ɂ?[
nHV2?ïÖ_ÛæMÛ?qË°÷êìÍ?=ÿq||x?E¡†AØ?rÿ'
*DÖ?pJˆ'¤™U?ïv+ÄBÔ?w44)›6?`u¬sƧ?LÊÛ¢H"%?Ž[ÉééIL?uçóæ_yœ?ï¿:֞:q?Y`
º¿Ü?T>WŸMi?9ŸÑ\´1—?{RþÛè?X•ž?ú?ïÁú°N«£?q-ï}'?Pƒ)vM5?GÉÅ-îK?zá݁Ûæ?p*Þ]??ï|-hv"?Œ¼vC–<?NJ/Çø=M?XµûÌ×ñ?ïƒ
?‹Ò$ñ7œ?ïkhT ?…,Ë°°?i"óøz›?a½EëNœ‹?šÀ
ïÄ?ƒ[Fe՝Ý?ïN^úƒ·?wŠƒýR2?hdµvðÓa?Yϐ´¶0?"!}sá2¼?wÕÂ;¿+AGN4FGL J0601.3+5444¿[`§݊ë@.=Ö[æÀ;7z)'ÉÁÀ<°œÉÏÂK@ Ñ6Œ.!&?ÿ€ì#ª)?ÉÝÂéI/?£Š¾ú?Ùb2z&@gï›û2?Ϲq%\0¿ìÕSïk]F¿¿c"OðÆ¿Û^'¢O¥¿ÛÞ9¿ëížÔkýAGNbcuGB6 J0601+5443?ïÈϺñ`³?ru"g*¶?@y¾N–?0¢ä3ëÙ?y† z—?r-4ZÁgÍ?ï@´ÄÕ÷?—p!€ü6?`ÒcI"c?g·]Åp£?•Ï/ÅÃØ­?–9Õæ[Q%?ïYŒqÏ}?Õ°ÑçV?\@—DÅ?X)úAPŠŽ?"
ýºB–?~Pñˆc©?ïcb"èjì?mKl›üβ?VaÛä{?9"&òbË?'3e•Ø…B?m8­ö'Ð?ïn³÷`@ª?=¬fƒuI?Q?¶ÎV?Džk}W1ù?'«¦ƒÚ?Œíى_?íøåñzÅÞ?¬Y°¸½ß?mÌh'²'?zZIü'@?®"Úbϒ?«s7¢\‹?î–<Ç}Ž?'°"~?aägš"™?QÆU)÷!?¥}í.Õ?'U"øü¡>?îä™óÇ?ì¡›Ÿ?k".Pä^»?Z+ é¶?­Xƒ|[L*?ŽT®¬F¯AGN4FGL J0601.4+2320¿Ó-CŸççZ?Íb±%&€À9Q¡/À;?‹!0Ò0@Ò.ϏÐ@#ë¤ÿ(j?Ãðç^HŠ³?ÊÛ9·†¿w?ÿãÿ¹‰#*@©5§¬¬Ç¿é¬¤G¿Òvǝ
"¿êçÓh'1¿èá?(‰â¿ç)\OŒ/N¿ïã²…AGNfsrq3FGL J0601.5+2309MG2 J060149+2324?ä¼(&‡¼?Àò½zõ??ŽqÌXÛ#Ø?…æö-Ö
?Ք!P˜Úé?À¢_:øúR?ßù¢1²nl?κè^M¾$?œ° ç"±? pR~?Þ;TÜȏÉ?̀«tk?äÎC¼»?°Hëï¤SŒ?¬l´3Mà3?˜™?óD
?Ô4+Ýʄ?­ðu'›Î?çè÷¯ú?¦&L½?^?£³	úw!l?€-ù»2?ËsQƒw¼?¤Ý	Î9?Ôõ¼ÏBŒ±?ÀL£mi ;?šPU†Xïç?'}ìÒÂ([?䲞ìGo?Àœ?hm3?ÑõŽ´?Æّݞ½V?¨liG«á?­%º0µKô?åö,~Ût¨?ǒ1ʗ,F?؞âÙ©?²iðËKñ°?·E 2LôÉ?¡ð‹²•ô?àÇڌÓãl?²V
V¬ih?à>"à"?±´úÃ"Ï?´òæfõÚ?˜X*KÉ^?ÚG6 ‰ž‹?²}bò€ MIXED4FGL J0601.8-2003?yïÛÀ3Ùä"sÀ::Ó8÷˜RÀ<L•òE,Z@±y]äâ˜@ir)Zl?ÀÏÔ©É?Áª~™8 ?ùA".öŽ@ÞR}T•¿Ï®2M"¿â°FŸ ¿é›H€w^±¿ì|¿8"†?§"Uür'¿ïýïŸ_¬8AGNfsrqPMN J0601-2004?ïãë«ùÝ@?r®"F.e¬?GßÆÜ>K?S?'Â?fb"­ö?oH¦R0Å?ïÝ)IÍ\?qòù‡—ðÁ?CB¾06¡?UÊó'eïÍ?nM'v<?m½‡A ±Ø?ï^–¹Èì¡?‡Å‹•ç?]àEíûf­?a¢ïäíë?'O$m'm?†Ô£}?"5?ïä¯ƙ#?N|W‡#4+?4jÝæ¶Ur?%"¢Ôm5|?hÓDJù?LúŸî©?ï¤)Î?Sâãáý'?hÄûÕsns?vs
rh*?€ÇûŒÞ¾?‰ÕØ!/HÅ?©™A?‹AlU½0?SØ֘˜Ì?cý+$Ì6?‡ÕzÒKjK?ˆÜxƒ¢Ëí?î´º~/t§?—	ÄÃ̚Ž?m{ôwː?p¬Ó7¥?¢Ü@[…yá?–..'ž?臭7ù˜?pmTAúº?Q°D@J¢?IåŒËóÞ«?ƒbé·ɕ?nEyr6óAGN4FGL J0602.0+5315¿ïŸ;˜m°Ä@-%åр´À9{ÌÀ7"À<+6
Ä@ÈÏ»i£?þùLVè?®°ÀÁj‡Í?œt2¬Ðƒ?ð'޻♾@'Áƒ¢?æZºÌH¦¿Ô€'ཚ€¿á~•Üär¿Ù5_Þ7v¿ážXæK#¿ÓÂùå3ËßAGNbll3FGL J0602.2+5314GB6 J0601+5315?↓þ¦8¹?ªxùÆ=6?.‹ ©<ÍÓ?_3•Ä?5'¦K|€?ªzN_:vi?ïáY¶¢
y?pw{	Rè?@ºµ?PQ®5G?juÇÙN4ž?kzµ@§¯™?ï¨_˜R-?w…¸™jô?VûùÖ[D?[‹_oÖ??ƒhà'î=?v"yÄh'?ï¤ќj?Zh;+8ã­?QöR-O"™?1=w-êHÃ?z0+|¿ž?X󺤺Š¯?ï»Þ´UÞ?€Óí…Òq?=_	ô?.ì`†`΍?€QÍa¤(?€©u¦À‰¡?V$i?‰ûà"Ý3?QÌßA›.?`P»8?†Ö¢6ì¾>?ˆoÁυÉ4?ïkG@}Àí?ƒ&ý֔%®?ašÈ
uÅÄ?dz;ç|ó?c¾ï©š?¨9¡_¬P?ï\+Æ=¢´?vòÎÿVÌ?h¥à³ŒD?Q|)þuv-?'eË#
ýî?tòk'¤OÒAGN4FGL J0602.7-0007?ïáÓ¢)
:À%»Åޜ*À:@x
Ә™À;Ê%o%QÉ@i€0¼áG@S7ë(Ø?Ê$ Eűû?ÃU6hFæC?ô²—,Ê@ÏÁZRÜÇ?æäíU'¿ÒãIüMmò¿éSe¢òð¿àÜ®ÙÄ­¿çãœA¿'ý¿ïÿð`OËðAGNbllPMN J0602-0004?뒎ZvC(?·'ö""ž?ˆ+Qˆþ?…ôÕ7Qn?À3~œVý?¶{þÁ "?èÕÞµÇ;'?ÂhØÇ4?‹×$b·Œ?øV{RU?ÊëâI¥?ÁÌJ%½ÿª?ê¦ØÙÓú?©
®Yé,3?˜4WC? ¤¸¢—?Âe
$:r?¦¤Ù†ÍÒ?êªOL¡÷À?"µ'nÍËÍ? <éñCü9?z\ô?]*?ÁGˆR§ö1?'nké>9Ð?窱Šã.Ÿ?ÁÙA@M^>?š xÇA;—?"'GÀ§Þ'?Î*¼0O?Á tmÿÑ¡?ãŠæpëX1?Ê´ŒA?M/@†ï"?¨wg!™¥%?×`*sWL?Éü¥zg>?å]؍A¾ß?²:ýk2ûk?§ÑAM=¦?™ƒÎ||D?ÒR4½nWn?±o	¦ô€X?ãBa…<P¤?¥´´ùH5?³xp§xxŽ?•FÝC™[&?ԝ Ì4?¦lû³˜‡òAGN4FGL J0602.8-4019¿Ôw"¨qUÀ9÷±ÿÀ9HÙè>B[À;֞-}Í@MË°4z?ü¨zd×ñ?°ûe€Q7ð?º‰Û
¨$¢@
MÆýòÿ@çÖøj¿ïá÷ ³SÕ?ﻹ.׿àƒËÑû	÷¿Õ(šž&q.¿â«¤(hÔÖ¿æ &5AGNbll3FGL J0602.8-4016SUMSS J060251-401845?ïȖ꒰q?lÄff±Mâ?X»Â1=Ä?Qœ[ÇMEQ?u…šû,I?g‹Åù¥o$?ï˜b–'ì?‡˜ë£ño?e£|N­?lýø&äc¡?"Ÿq‹7Ë?'¤\sÑçq?ï#¹Ÿ=Z?Œúó''ñ?yøސAø?{çÁ]îsÂ?•
ÆÚ#àJ?‡øú#Þ[´?íã>‰0H?ˆøµmf‰?‰Uì9¤'?hY¯ÁÊ X?«yD:yS?†«i$ƒX?ïmT?†‹B?pG‰ìý>?k%Úşæ?Œ™¹"k§Ó?é}Sôd?îÓ¥¦d¥"? "
ú¥´?|@>O&r?Š@2è€?ž{Ikf§ë?š'c3?îJÉ)ªu?šS$édI?†¥×Ûí¨Å?†"¯
Ôg?¥©÷o>¥x?•)ˆï»)Û?ì
š(=iv?žìFìvÖä?–eZ¸Ó?yéøÅ	È?ºØ7—?Ž`K1f0AGN4FGL J0602.8+6041¿å†¹'³Kq@1ÒZh+b"À;LN¢ûB+À<›—¸
@çט'Ã>@k¦ý/k(?ÌȆŽàÙ?·sÞt?î'ÿú Ã@p ó•Žr?ïØ+oðRä¿ãDD¾ÂH¿çÂ>hñ["¿ÝÛ«aïÿÿÊPË?ïÿý¡UûŠAGNbcuNVSS J060324+604009?ï¦{€î–»?•[ÞVè?cÐ@Õ@­?_nÇ¢F?mº=—%?"…âT3ãü?î՚˜¿vo?¡NL¡ë¸û?…04	δ#?Œ¡£f¸?š´'Þn?š0³%Í?îôÖÆÔC?Ž%^^Z(k?"Ì·Hï«?…ÁJrù?—‰>PR?…ê¡B12:?ïÒ* ²?y
7Ÿ}+?vÄúÇb#é?\ý\š´C?—4~ëK¹?uÖ£®z
5?ïi]oØç?ŒÄÖ¾{ï?q(Ó0…®&?o*Ê@AïÓ?:osŠ?‰s¡p™?í0}'f?³ó…Šá?"sR)è¸?žVÅßrÁ¾?±Ÿ?bûÔ ?¯®u?îVG+Úò?™¢)0?Šjya–?…";ä\¶d?¨¯ý4þÍA?•ñj܄à+?ìŠ5z$"8?šs'tË?"Aᯄ}Ù?âªÛ9×?¶ÝÛÁFÌ?—ŠØêçgAGN4FGL J0603.9+2159?íU`U³Ä?¨˜,C;À9g l‡ØÀ;IéÁЈ@‡T>7É@·a*½C?·œ8°J¶¿š€)†G\?ãA® 9[k@	 ˒:*?âÁ?/À¸¿âÀ+i:V=¿ë¦¬ÂkIû¿Ñö0‡ÿ¿ëÄ®…¹èÄ¿˜èíû׸tAGNbcu3FGL J0603.8+21554C +22.12?ìàåҜy?²€XèQø?plÍêùB€?kÖÛ.êm)?·òŠkbÖ?²>ŽÑôÕ?çàð³[â?ËiGlP5M?j¡¹reð?…oæïm?Ð܎re?ËLڒ÷Ù?ë¥WœÙŒ?§TáM;?"ì!ݽŽU?jia_ÄË?½š: ²4?¥gÜX+O?îcFæJ?‡ÆaD?rÚÑ>Ã×}?Vó2MkSò?«ÎqiYí?†-š›`éÜ?éf\W½}?À#<aÕ?ƒ÷#&d‡ƒ?N½xtÈ?É'pñQ3?¿‹·"èk?ãÀîùƒ D?Î`Š}áœ?t­Ô1˜šë?ã¡Ø°Å?Ø+j¼âI?Î<á¨|?è5œò-?°ï&œ…¥?Ÿc…ª\1?•S¢£àBÁ?Ë=ƒ-
i?°€)€Â?êÍj÷;^?¡'í!mc?|¹&6Qt?zŽï´:Õ?º¼ÿÐ/X? ÷NG	¥AGN4FGL J0604.1-4816¿Ö[YÆ"—7À;}Oß;dZÀ:‰øg…JWÀ<|õÎMÖM@!SCÉÙR?ûêï,s%'?¿÷>….?³Íï6¯©?öêºÅ­@ú9lˆ>¿ï°OžMÞZ?ïüÅþ§e_¿ÜÀæå|ǿ܍üb;´a¿ÜÕ9BkàN¿Â¨Xú2ÍAGNbll3FGL J0604.1-48171ES 0602-482?ï踙Ë(ï?~ùþ'ˆ1?3®³Åd4?GýñM?dє¹á9Î?|	´<7?ïÙÐ¥c@0?p¾Šìaûc?=Û~
‹ð?E½Ån(u#?q9õ""ýB?n
ÉÖq?ï'/)®ƒ?Fo¬?UUÍZDþº?aºÙói'?ˆÉ…Ôò‰k?€ÖþƒÅô?ïv
÷]w³?jØ]ú‡;?^Ûµ:ç_?A¸j/ö<?Ž¡Ë5cf?jð0Ù¾?ïلýÅ?n)U¿õ*é?F³Nٞt?B¦ä+î{'?pglÕT©?k(èUŽ,Ì?'²Zí?…•éŠ€?Jú˜!sg?U'Õ5Î,?‰¦ñÊFÛh?"
åÌV?ïPÌ'v©?…7¿4ïc?YB÷)Ê+?X_\@ь?"RZ‹~Þ3?"öMŸ|#ë?î"Éлf??‡¥(Ê͹Ê?q<aÅkÔ??^öÄïêþK?¤›Ö¿ý¡û?‡¿cë}`*AGN4FGL J0604.5-4851?Ò­Td¹Æ"À;‰¹"¬TÀ;5£ÇeÀ<šó5í"@:^}¹¿)@{\ÚÌiÐ?Åícۜž\?‡5ÖP¯	?ÁÊ'˜˜"@ftá~_¬?ïõœdO4ñ¿å›	Ü!Ôf¿éë‡ç`Í¿ÝÖÚhµÌ¿ês€€C¿»4.A2³AGNbcu3FGL J0604.7-4849SUMSS J060433-484947?ï—'ÆUS?»ôôÍá?]ÎÜç!·?ƒi'âNe?špø˜Ø?¹Ó°ù~þÛ?ï³í7ë?{UsÁ#?SÂ]''¢?XèT§G
M?€Ä¹Ó#?wK
R¢†ø?ï=хª_¡?ˆùÂó0îó?c3pŽÃ?T›äõ¨A?•ßaNúd
?ˆˆïK~â?ï²ß "þˆ?]­'š²ù[?Rä"ÁüåÈ?4)¶[iÎ?€ë¥<©kV?]ank€Ê?îðYÝÄ?±øñù?hOB­)'o?nÉ͸µáŸ?žöƒ"jM?±¬vœ½2?ï7è­º0?'ïcן¸?aõÿí©ÅÅ?kX5'[S?–Ä*I§)T?'f –.P?î¸
£Lÿ?'%KüÉ7ï?m¿2»S}?nUêê°g°?¢£=Ïq×Y?'5u}Q?î͉á?}þRiíw?oY|]¥¯?V_Nae_P?ž!Ÿ²ÄU2?~1ç)¬ŽAGN4FGL J0604.8+4411?ß/썲[@%Èù±1eÔÀ:ecãÔPÀ<Ȓ«hÏ@:"çÛÇ@oê#èù?Ã×ã–½Ç ?«M-5?åŠgAؒ~@˜Õl²?Ûú"•üV'¿æ»`(^ÃÛ¿âèìô,¿ê§Š$Ô¿æ²^âc¿ðAGNbcuS4 0600+44?祐c	å‡?€Îñõ»*{?T;ü›t¢®?G£O¿?ƒ§¶«Ù?€KG,#?ï	+hʪð?¢¦-Kž¬,?bë`mI?lèFÔ9x~?œ}"¹•æ?¡Ô¾{Ùȼ?ïÍ2• ?‰¹?cK?sNÐ=ÆK?sëÕÙjYÛ?˜²ª*Ä l?†M/ìSf4?ïcK_,"å?hû¯ÐõöÇ?gJ€çÑø?H7*ŇÕ?´JÇdÞ?f}æí¥Ù?îô/lT<?«wÐkô·ü?j†99
y]?rÒ(0<µ?ž,ræÄY?©}	ãP`?í›Û«ë^f?´Þ»ÂÑZØ?x0á†Ü•O?ø‡žký?±ž†'~?³¨¿%À?íÝé
äÞÖ?œ!Q´R­w?ƒ8b^Õ?}§Ì‹×½?­:!5ã?™Y¼ÝÍT?î6°õ?…æ[vð¹?€†QƒÏY¤?gb©ê!Y?¨rIðû/€?ƒ¼¦ÕeyaAGN4FGL J0604.9-0000?ï U'¤´«À$§ñQçSÀ9Ö¡Š(ãNÀ;ëŸ+©Ñö@ `|°Ä®?þŤðñ5?ÁÇÓ(["Ð?Àöh½ÕG@Õ%`â™?úé!>"l?ȏËåq3t¿ãP´î‰µ÷¿ÛžgŸ —$¿àÕß?Á#¿ÍÎùÁ¢w¿ïÿú Âî'AGNbcu3FGL J0605.0-0000GB6 J0604+0000?í=ц3Ð?ª\éΰê©?ràÈ•«ô?l?Pôù_?´ãgLæÀ?©Ü"o?éæÒ;:'w?ÀQӒ†!?"-{*œ?ˆEÒdi˜?Ç!ßa,žL?¿®¯*z|ô?í\ÓÖ«?œzÜQã?ŽåD¼Y?‰°LyÛW7?±C@ÝWîÛ?˜By-[?éØ¢V=?˜°éT]sz?–·v|È£S?z¡SÒ¹›?Åƈß{êÌ?—°¤—hæ?ꂨeÜ !?¹úÊeX8??Ž/ÕDel?ˆ@†¤é´?ÄËlƒ¤?¸n³rÛ?ãT»ã½Ìv?ËFMó—¬?–Œ;$RÌ?úðÓeŽ?×íĆ#½l?ʜqãû›?ê¦õā"'?¥ÚQ€âNÐ?šO"I;¸\?á­i/ª?Â8cQf®?£ÁÕ\o?ô?âÃÜcÌ5×?ª®ÌXIs?¦~"VhZ?"jÜeó¯"?רv´Å͈?«'ƃ°AGN4FGL J0606.5-4730¿ìßÄaøÀ:ò|ᛑÀ:iƒ¾f½À<~)gØVn@¹_÷·\"?þSó?ÀgX>Zƒ¯?Ä5â:[€@Jb#ᆘ@ÿ8¯ÉÝ¿Ê~ÆÀï?ï†va[9¸¿ØBµ<u¯¿ÛlÛ z3x¿ã'ÿýPοç¸u'8)AGNbcu3FGL J0606.4-4729RX J060635.9-473001?ï¦Á^ÉRß?±5ܬX?XÃ_¢':¤?s'½5ðǽ?ƒ7<aðü?°ô)ytUÕ?ïÄçL	?y#–"ÿ•?Q=Oþ…U?WP8ØѸ?y¢8`,B?t³Ž+/ì?ï¦ÂöE}I?s}˜8ì?\uº£žºõ?bD%lù?'À‹îu?p«
üj8Ì?ïˆ lÔa?q½'Ždߌ?{yUqmI?YQ£ÌN}â?•¸µ³"?oÑ£x?ﳀp'Û;?!pà2E?lÈhnœG?k¥Q¨¨!?wÛÄ6{<6?v@Pù|ä?ïN–ñž"T?â¥Ú?cvÎ!cbˆ?m+Lð—±?"¾H
ìÔ:?"n_LR?ï]3½ÔÈ?X:®n";?kÝYqJ+?oá|zۃ–?ÝÝ>ª¢»?}﬽çs?íä÷/Ä5F?Œ-"³ÞˆD?bf?tÒiA¸?ªk4Z¿X	?ˆN¾fóù
AGN4FGL J0606.9+4402?瘝wÁúÙ@&SZBkµ[À;ˆ²køvŸÀ<¯
¾Ÿã`@"vJâ§T˜?àÖ`ÿõE?âÌ|ý?ïÿÿ&¦³@™xâií@žÔ2FÏ¿ì?2_Μ±?Ûìû@}ž'¿æïa¢1n¿Æ`¯Z9²?¿ÒČ¿ïÿ̞©£ÓAGNbcuCRATES J060650+440144?îä»)DG?¥Êyه[¯?‡GVBç70?œ@Š'Äf¸?—ÄóÛ©†?ŸÉ(AV{?êÒÊ®2ª?ÈNr…>Ôã?Š+(_¶*?˜nZ«¼¿?Ã"À&ÿ§?Æï¬!þÏÌ?í‡À¤S£? Ë¾1óq?¡%ý{ÒoŠ?—Ï·G[\"?¦]ø@´t=?–øs6?í5ž+"py?¿)8B¦?bh{z°Ü?eòñ>éA?µÂó^uÅï?@úìR?íþ"iƒý?ª<ÿò&?ž'³ë+<?¡šð¨;vb? ÖÌÃÒ"-?žÎZ7+?çeéÂë'?ѱ%y-µ½?™?WWŽ ?°¡uE9`˜?ÏCùmÙf'?Ц«U[?쭑ߢ"»?¤	·œ÷?ÖN1ºƒ?—®³ƒ»æê?³S;mª­‡? LÒéïQ?éω?%Ò?·Sîgޖ?eHnÎþ¢?t6`Š?ÈlºéJ†â?·J]¡ÒÀZAGN4FGL J0607.2-2518?æêÐN^ïÀ4mÙ ð¥ðÀ:ñe9?¼®À<­¢pØ°0@ Iý?üÿ¥·µ
"?ÌNÖý¨7?ÒûG¿1X¾@*3<m@î" ÞÇÌ¿ïÿÝÑô?ïòÑ®³Ý¿Ì°B'—É‹¿Ô§â݅W¿è…ÀsοÆx øóò+AGNbll1RXS J060714.2-251855?ïÈљK|?®eÿ£¹®?VQàšLƒz?‰£YC٘?v_%"Pâ?§ýŽÀŽñ?ï±(³lBb?wD°-
?^Ȉ¼ÉìÀ?fôÿ¤Š?¹"=k?|n%W<yÆ?ïC'üÇf[?Š&å§L%A?tOÄ͝¬Í?{T+ü¿Ð?'y¯5»Z?…z‡wÜo'?ï)8…Ç?q¹]@ç=Ÿ?€k{§×Ò?]<PÜ
µ?•Ȟõ?nµ&$óM—?ïÎXÁÉIÇ?k¤'Éfö?YçQ*‡'?O_óþ~áÑ?rYÊ䤶¬?g$; Ïò´?îí3ˆ(ê?ª²[a™…Ê?yjk3¢ÀD?Š ùùy@?œ~Ɖ°¦?¨}xÑKW?îמðN:?'­EA)uW?z­a½¬=Ì?€~€ù¹?žqS¬ç\?F‡¶³©è?íâr¾<?Œ-­9?	5Zk5¢?vãá2×»
?©Ô9oæ¬m?ˆ-P×D0BAGN4FGL J0607.4+4739¿ä"oLi@)»ZBkµ[À8KÅPÉÀ;‰†¶hz@hÛ!yL?ÿ묋å?Ÿžöaù?²î˜àJd@Éé^ÓÊî@€9Küï?ä·¬ÿýѧ¿Þ­€×*ô ¿ß–7D9ë´¿Þ9p¤'Öµ¿ä,™¦5¿æ%¢HZãAGNbll3FGL J0607.4+4739TXS 0603+476?ïáàŒXz?`Á@Ì«Ä.?@á²ñøxa?3RmˆÇ³q?j)²æý'š?_f"·GI?¦Eq?ˆôD'J?_¦@AFÅÚ?f_:ÔC~?"…Pkôò?†¡¹¹†?ï«AäÉ:>?}^¢K¤ƒ?_'c÷f?fìäêT??:QÜRé?z£6þPFÏ?ï>䛏Vä?qDˆù–âä?q§ËËÄß?PÂ4"àjd?"á""H?oº‹4±¢w?ïÉõ¬êÚ)?lÔÒž?>¡Ì
©?2áó^ïÀ?yÍ 5Q?l/°‰*¤¯?îðîr=?¦u¸™'Ê?v	,B?ˆ6w1ü¶?œ|·.׎/?¤…9'xpÓ?ï"¸QsC?‡ö«"°<?lŠ½@çHž?yǸâDcH?""™Y™)?'¤;]Í_?îE‡,?à&?"c{ˆ3?'4%õn?iŠx€lé?§ŠunA?‹0%´/ø	AGN4FGL J0608.0+6721¿å/"ƒÁQU@4ßH!ÄvÀ:É¥Ð߁À<rÁÄN¯@Ô®rC¿G@e²€fÃ?·_ïÕ?¶O•¿ol?ýŒð=ë@‹ëëv@?ïþ¸*¥¿åڀ¶–*¿æšmÔﱿç
ýQúÊ¿éOt¢>XÖ¿ïüßÿÚkFAGNfsrqS4 0602+67?ïñùé ј?QébÕX@?=|7²¹¾Z?HôÈÌ7Z?T­ ZK¤'?GœÜF%?ïßتümy?o}Im6ƒ-?F÷àU‹?WX¸ë–?ji\÷ee?hýy
½?ﲦ†i?nXx=†¤Ç?^•øV뭎?Xª&Ï4?tH¡?jÞø™êWc?ïãÊ\Q†þ?IIH-[?Q"oVϘx?3(Â˜?ckìï-þ?EN.±"?ïã]¿Æ ƒ?`ûØ?}§?O²Ô…ÎbÔ?Q Þã|É?dµ‹(ÆÕ]?Z܁—
›T?ï§|4?ä?†z™"µ0?W('Þ÷±¥?l†Ê0?ƒ;â ÈÞ¾?'ó.ll=U?ïnc–0>?ûÇ¥ˆG²?pê@¾rª4?už²õ ?‹ñú	Åk?{ÐPHÅ|?ïªÊfô‰]?iÏÖ´žô?kx¨þp–?T™ÊXj?|Þx"8ù?dÊt|¯v AGN4FGL J0608.0-0835¿áX¢X…À+-{cM­À8z!ÛòÚÀ;gUá³äž@Vä£-@ÝÛ?VW?§ åþ¢û?²#ì€ÏÚ@M­àx{<@­þ/Eh¿É]úºpª¿áé1â¦'ò¿å¬¬›ÔÝ=¿år|õ$®¿ëÏY¿Žö¨¿ã‡%Ž/AGNfsrq3FGL J0608.0-0835PKS 0605-08?ïܶ
åé ?hÀînÉf…?@¢3€Ø=l?]¾SÍÞuç?o!e]âˆ?bŸú¬‡?ïíõ©ÛÖ?fX¾cL³f?/©¨b+??µùuð?`ÅM-+œ?c¹x"V†?ïCZ{w?'?Õsˆ?u&æÃËÌ?U›õâÃK?'\äZÓ£:?ŽdjÃL?ïßMdP¦O?Q5:‰«?6Lê'Ó\? ¶'ð‰?mèþ,¨kû?P(äA€©?ï›Ýû¨?ÄÞBHV?Ešcfm¿ß?9"›[b?‡®Ûüý?€½°i5?ïÊZ€˜Ûr?†4íÛUʺ?M¶ª#Se?n?ŒÞ!j?wꄪ1Š?ƒÚýVé'?îåßØÃ%.?˜Kc«¡?'η†"?‡Ôȯæ|?š6†>A0?"B°•
â¤?ﳀ'$(¡?l'»Ê'¶?M	Ëb%Šø?>Ad³ž?OYuº[Ï?jÅmŠU"›AGN4FGL J0608.1-6028?è:ñ"½aÀ<¡ð†nDÀ:+>WS£ìÀ<
¢"ú¦$@Þ)=Ðñ@T™Â´E?ÅÆæXäóŠ?ÇU¸a°Ê@¥á¦x¥@Ô&Z²©
?àî姏&¿æf¬![š[¿éq+¼FlÌ¿éê šª;¿ïÿøþÙå9?äãÀEçAGNfsrqPKS 0607-605?ïòb'¾«n?N€ûH®û?DÔVGšI–?A—V¢¤û?PЯÄJ¢?Cùq­Xñ?ï¨A£AÓ?…w>©G)?`þÑ£i…¹?lœO±0ù?¯âÑÞéâ?€óßÈfY?ïŠv»jœ#?]¨bAa?kµL5RÀ?n±5Ž¢…ª?†tþ&-ˆœ?|+&"]?ï©×'ª?dpaó€6ç?`'†\qa?BaÄûD?$?…{ûJ?bØ/\´ñ?ïçj
ÿ‹Ö?[Ðeê/Ö?U7	l"c¹?NÖÐJ½|?[ôÚ+àэ?RvÓÏÖ¥?îöøuOÀæ? 8~º"Æ…?sû¯É¾ÈÑ?ƒÿzIýã?œ"^DÌ?›L¬ÃýLE?ï+†	ޔå?Œ¯æ¨b?{C¢¾¿m?z¨r+iÛÔ?"¾x#¼Ãv?‡^Z†çÃÒ?îµÑ¬–²›?‡ÅHIúR?6\ÿþ‡?hׄ0Z̎? ¼"YFv?†:áoAGN4FGL J0608.1-1521¿ã~GÐñlÀ0aóFí$À9²L‡À;ãIâ¢!@ª<ANÔÏ@aÏBÈÒl?­Q4¿¿	?µåê**ËÜ?ÿG±õ°ñ¥@ô÷ή#i¿ÐFŸ ¿â-¸À%t"¿é£€}"Ô‰¿æ5v•ˆ"¿é"|žâê¿ïÇõAàõúAGNfsrq3FGL J0608.1-1522PMN J0608-1520?ïøÂÐZÝ??¨`)üc?'M͕!@Œ?Î(7œ?G!K6i@?:…ç?ïð´6햶?c†À–Žu?$ÄՎTü?4ý[ÅòÛ?[þ÷ÁëæÏ?b…¶Ž6?óÉß?y°Àѐ±·?cn5¶ñ
?dÉàÄ[{/?ƒ=5Õáà?vHi0\G‹?ï÷lñDü3?3¼Ë
'9?$!
·B'¥?
wñÝòþ?MC÷w÷G?2L—'ŸëK?ïóCcN{[?M¶úç¤oG?2u¼¦T4*?&Р™€]}?TÛÉÙ?.d?J':Â!Z?ïÐE(?'7)³gÖë?E_9%z­ý?^f¼éPO?uQvUùÜý?
܀Â#?ïa®ÏÇå?†ïêØ'S?qä‹KøLë?v2t™÷aÈ?Ž¢g² ?¬ˆX"s"?ïèéy'øw?TŒêºÃ"??žLVí&j?1^[ÖrÍ?c"½?Q°	°ssíAGN4FGL J0608.9-5456?éo-&Æ`À;Þâ¨dªÀ9·CsóãÀ<^ÄÞÁÁ×@Û]ˆœFG@""³º­?¶æPV"œ?Ø*ƒ·/,@ö"aKts@[ûÎíäJ¿â F\㕿ãíÝÞÂî}¿è\…qÄhz¿ëZ}ú×¢¿íÓø:8á¿ðAGNbcuPKS 0607-549?ïñf?'ªr?Z·9Æë›?Jý2–QÀG?P_̶'…‹?OiÏÕ7‹?Lš•h~Û?ïÝ–Ý…4?rr'—Š!?Aœl»Ÿ½È?NÎ(ˆl'²?nMݕ\G?oŽ^
b¥M?ï¨úå[[h?|¯~†Žg?fÙÛ%o™?r¶õ2¼&Í?€
Ïïói®?wh?f=¾?ïè–ó³&Å?H:é†5²#?R$­ŽäùÛ?83Ìu¹ý?\­j—Zƒ?A=ÇÔÙÞ?ïì/&ée?U䐏œ?RàQß5?Fí­‰ H?TÁcG$R?M@ɲ¡¿?ïRê?è¿Xæü?XµÍªõ?jÄQ"?‰£Þ O?@²r†Ê?ïbÉ¡§¸Ÿ?†W`
ü?q´Dʛ(j?wÇ‰>?Žsu3+þ?ƒ:ÃÛlŽÓ?ï¿Yx'•,?hnC2$?jQï÷Í>%?X¯zW88ê?s*KÑbOU?a‡ñ-Û¬£AGN4FGL J0609.0-2219¿íTÊM§¹ÔÀ2ñåÀ¹™À:ãêÀӚFÀ<x
œ;4‰@õ¨ä_@'‹vÁ?Ò:og–è?Õ£(c¡e@°ÄXŠÑ@	ªçŸ¶ê?äEôî¿äb¼ÃjM|¿ßM<+¬¿á¡4x­'¿êƄ^I¿ß·$¥Ñ¶AGNfsrqPKS 0606-223?ïÂ)âá ?o8è×÷]?Z]--U?OUx#ÒEÑ?xSÍÙ¦rÆ?j5ނX"ª?ïSO»Ýš?…æ""R?if°°+íG?røJ\£"?…'ï¤h*?€K7DeŽ¾?ïHο¯ó?Ž*ª­Ðù¦?€ÐQÝßkû?€œ©É.‰?•N½3nð¸?‡À`ŽÓEv?îø!çÜG¿?sÅæ*£?pmO|k?LÔÒÊqÜ¿?œà|-Ø=_?r¼I\îU!?ïËSÔ?€±ÊΩö{?i]½&­?_â+ÀxH?†5õ·%s?}
CÜhî ?îôƒ¹f?žáûû<
˜?uymû‹E?"rìßLc?œ©5x»?šQˆóÝr?î£Rr"›S?"¼JûO6â?†"דðÐG?†^Ht]Öè? )¢ðHÃ?Ÿ0À
âò?ìÐÖü?oñ?'Z
ՐÀ?'ö?¹0¿7?i¢6ø ?·€'æJŽ?'0Å\ÐlhAGN4FGL J0609.2-0247¿ïʋDþHÀ%Q|=h@[À9‰PÉSœÀ;Êrß­*@ 7QŒºŽ?úºܓn?¸õÜ»'M?LJeºnü7@«3¥Cò@˜¡˜–N¿ïÿC*!<?ïýûþé‹¿¦`ʛK¿ÔŽUëæοÚbX"üS£¿è'kr>á½AGNbll3FGL J0609.4-0248NVSS J060915-024754?ìW¸^^b¿?¯³z³}Úò?¦V%vh.k?œôÁÄl?²*S"­M?§µF³Ã'e?îÏC¢A2û?¦f¶f…¥?'"ì5pÃÃ?lp³Ê±å?œÍ–Ã?¢mèÔ©àÆ?ìC¦\íä?¥;º7—ô?£½*?™K^Âì?´
Š§ð<? +k—êú?é"¡CB[?£Í¤ùî?¿¥)Â1˜?~>+†VöÑ?È1¼ÕL¼á?¢'Іþ|ì?è­µ)÷€?»s‰uÆ<?¶ðüÿZï?ªÞÖxgÝÄ?ÂC2ÞéHÈ?µ
UÞ@Ù?쮼.L¢#?»–¹â±²â?šô;¡wÑ¡?¨:¦!ŒC?³Í¦†Õ?·{<iVú?éÒfv}I?©ª€±;,ï?±™4ÈHS? zÍ2š©[?¿Ó—†Û/?¤\ˆ¾–Xe?ãßþž½+*?±*<óß÷?§"óáej{?"íïpáu™?ÕM"Fö?±Î´¡fžAGN4FGL J0609.5+1402?ãÊ­úí$À&ü›ÇqCÀ9¼ˆ\ZsêÀ;P°Å/Iš@×r'¦
@.—ÂÿÄq?Ëaë¼?ÍÍړßÆ@yŠ˜?ûptgÊ?ïkcÉ€?Ñ´GDãù¿çt÷Ãñ[ø¿éxv¾ù$š¿ãºàŽµ:¿ï÷šÁ6ì{AGNbcuNVSS J060922+140744?âÈsž©Ñ?½.ÛúV¿?z´'5÷I'?q–4æ`Ï}?ÚF¹ÖXš?½ךÜß?ßñ'ÌS‰?Å1úñDÉ?šÖ´B—s1?'µµ#ÐÏ?Þa})\«ä?Ã'àC¦?äs±́?°€påC±É?£çXØÚ?'´ Ž³ë?ԛ²½Eßø?¯a€†IÇ?á¸|=	Ã?¦Ì®˜y?µ˜ë8ÝÒ?'c"'Œ~?×(Ì¿ƒ/—?¦13¨ÉÄL?ÑWÜk·oT?¸•ßIØåU?‰ß+ïÔ?€j ™Pf$?æïöM'Gv?¸œN»s	í?ÊÛ¦lÄW?¾—Gü?¨`¼Ó6q¢?¨¦rJ>Je?çÃ
—ľr?À½Çå÷?Ö@[ÙßH¿?² à=–y?¯½]¯b͍?–4 *3X"?âãü8l¥g?³7'ÖÖ€?ÓøމÉÔ?ª_k6Œ?À
 w¯9?¢Øi;hË?âyÛrÏLÑ?¯9êÁE2MIXED4FGL J0610.1-1848?êÓzóùÀ1Sü¹#¢œÀ9Ü36ÌEÀ<(!à$˜f@Ž±¥ÿÙj@SI€C‡?ºbe¥Ì,ê?¸NPº*?ýãGG½-ó@
âmúy-¿ïΣ Öå*?ìû‡_Û1ê¿äßzïŠf÷¿åu{aöD¿å©ø¡çÆοïÿ"ÞïAGNbll2FGL J0609.6-1847PMN J0610-1847?ïð˜)kš?MIÖ¥Rç	?0°Z"pó?!âØR>»?ZÊÅç›|?K
ã6Ãâ…?ïßWˆŸm»?tڀ¿+<?A®ttú©¦?O:à­mˆ?l<Úm¦Â?r/KZ»õ$?ëî%7?}zøÅR?fÕÈŒ¡&?q«aÚÈÞ`?ƒb"	:óè?v7òð­é'?ï¥ÄØ.*?^-ªýu?kÝӑù™?L'ÅåŃG?/˜Š?XôšTS6?ïÞy[ûBE?aÅÝÀs!?FùF^Ç?:	—˜ýɨ?l%¥œ(`?_Ž\–-OV?ï²¹£zC?‡†gºS¥?VÃJhì?ko²ŽS?€y-È£
?"¦\±?ïSuÇ=§ç?‰VºFÄQ×?v\€â{#O?€rÿb‰¡?ôMÍÆÐg?'?ötïË¿?ï3v_,á5?yb½, ej?¢«}Õv?hBwo?'¨‰AIÛÈ?s¹ò"|'VAGN4FGL J0610.7+1656?¬{ïñ‡D¿ð%Q(ÀBÀ9&ÞßôǾÀ:ù^³ê}¸@ÀØNá£@6þ.n¨T?ÏiE~d^ú?àó°0´Ó²@ê¦ÒgA?ôWTБӿ̼°à]"p¿áO^AÔ¶¦¿ê¨ªxäî,¿ë6Èéé¿ð?èÞ¸AÐYõAGNbcuMG2 J061020+1701?ÑÿڊiiÀ?ʟ2œÞ.?Ù£"%ç?ÑäîpzU?Ôì'Sp¯.?Ë-"MTqœ?ÀŸ¸ìR?Ág¬®ì‰?ÒãùŸ]9?Ä"Fµà»Ü?âf]µ<ã?÷'‡ao?ÜKQnn?´¥N;áÓP?ÄñNaaï´?ªóØÑÔ#?Ù<FÆý™¸?´}Å·¨Ð?¯üÖi~Õ?ÃèI@jó?ܦ
$_õx?¯³
÷<Ó?ßZ[
ËMN?®…qßåZ?ÉҒ÷#&?Âg}Æ2–?Õî	Sœ?ÍÍU³»®Â?Ý(­øeÑ?ËwZü:? Æú2ë*?«Nt·tçW?Õ¡è
"ú?ÊÜ÷gU#É?ä"œU>S€?Ê]hPve?ÔTèþJ?²Fœ|M'?Ç¿e6¡¸Þ?¬{‰(×;?ßÌ2{°Ù?³édUf¥+?ˆ c&.מ?rµUæœn?àÿäÒ'*?¸:w'oSÍ?ß6ý³«O?·ìÒ[VMIXED4FGL J0610.9-6054?qgTÀ<TÔÜeÇÀ:Vªñ°±äÀ<%ÚV"K"@Ës0yE@|#ßÙ?ÂMò?¿1ãÁŸ¶Ù?ø¿}Xñ3@
5¨µv	¿æ5(¡ù¤¿à	+ÝÔ\
¿è'Bbûù¿èG"žy_¿å#—´½¿ïÿ¼C͈AGNfsrq3FGL J0611.1-6100PKS 0609-609?ïùuøîƒ?P]m{¬2?#òD"h8?!Jjt½Ûs?E/*­?O{ì9k‡ì?ïdž5}!?tÿòW5œö?I¯St¸í±?Z‹rz
?yúµÞ1Æ?r'°ùL|™?ï¦É ûì(?w›w%Œ'±?]ªõ£æè˜?iýR­CV?'˜9h'?s>¿¥gC3?º²3?e';ì´Û?^*á¾î5?AKü} †÷?…ÙuGlà…?dSÛô+ç2?ïòpeÌ@>?SYe
Á†?6'53Ò?1¡—ò©ðõ?U•g:ã´ý?P"ŠA\½?ïZ§À<µW?}­áøÛ?Y ÖÀ½´?`®å¬ÿ¿?"µå}éR?UÜ<?ïV€9m¬M?†´²)?e'Sk¸ç?`}¸¨ØšÄ?'Žâ1¤B?…¯<HpÃ?î¹ig;'A?…¨çxZÿ?ycÐêÕª¤?ejæô°\z?¡<ïpKþ—?"½3YrAGN4FGL J0611.1+4325?ïëÛäJu@'"ãq*À:ù»9À<Bˆ4ˆ@ «*èáÖI?û¬½³TUÃ?ÀA+‡‹O?À`Ò}»ÂŽ@*§Xžý‡@÷˜OŽ?ï9Õÿ{u¿㒰qLsv¿â}§Ë‹"-¿ÍzwëI¿ßõu|Y¿Û­A—$AGNbcu3FGL J0611.2+43237C 0607+4324?ïªá®R±?vNjˆ=]z?T#Â
|´Ê?Hhƒp¿%?'úWë18?töYÖ8š÷?쪌uï›Y?¹óVµ?€É(¿p$¢?~¥ÉË	??¸'w6¼Vg?¹\ŒÊˆ?îùèIˆ'¿?†FÕ>´x?t¸49"ò?t›(¯0œ?›"é¿Hk.?ƒ³ë)¾œ?íŠ}¦?…E‰®f‹?K-2º¨¸?moóœ´?¯:a—<?ƒ¥v½è«•?ïV'ûâÜ?….ßuø¨é?qi$–¶q?höÄڝji?äDÁ-º×?'†b.ò$?è
s¨e²?Ç3ÌÉze?™fVëä?¤kµÑJÅR?ÌVÿSS}?Æèlw?íæo°3†b?šÞËwe§?'D]Áhøâ?|ßðØP&Ê?­퍡8«?—oYUû˜?éÏ("D3È?ž§Y÷¨?£°X²Oœ@?Šßwãbý?Ã×IIíVR?œZ-Ñ}ZAGN4FGL J0611.6-2712?³*Ù"­À42®žä\6À:TWLíï\À<~vQ•ôÉ@®Š5x‡Ñ@HÜè£Ã?ÂE³ÆkŠ?½DÙMäa?÷Và·e\@¨AƒMÓ?ïÿÂÝ_¿åeƒGG½.¿å»;ÀJˆd¿äꨠÀ€¿ð?ï©·¸iAGNbcuPMN J0611-2709?ï×™۟?bhNÑ9?#~`RF~m?(a¼Ð®ÃG?sÖ@€#ã?b•¡gnN?ïêº_¦}?iý–œ£µ?2
W_Õµ×?Cî‰röeÏ?cUEõâ)?f~™ez®Ì?ó››?"¶ë/?ikv4&… ?u&¾ÏîÉ,?ö¥ŽôgÚ?xX4¨]í?ïõXÂÂes?6û¸‰a¸E?,º2áq"?¯Ò¤ˆ`?QËc[,Š?5f˜ÜÄ®?ïÒ*ÖÝ
Ì?{ïÅCmGi?1ÑDË5ö?6Eö‹j:9?ù&°Õ?{âqMó½?ïÂRŸ×m²?Òõå~+?F—'Å·?]µpˆÕÜS?|o %çª?€X$ßQl?ïk©îÏ?†â–þ)?p×ÈgYÝ?y0Êl…a?Œ°±\Z©,?'GN4ú?ïÝP"žá`?[Ú/.¯?EyVßu`a?5x³y£\Ì?mQßô©?Y1ã'YA¯AGN4FGL J0611.6+2803?Ä´o
YD@Ð]{ZÀ9ïËñqÈÀ;Öè`·Ñ@õÒö\")@æuš¶Ð?čaûÁ?ƨºžÌßA@ÓrSÍÝ@ʺˆýj$¿à4³eó?Ö÷PÄh¥0¿ÚÞŝ®|*¿ä2>@­o¿è¬QéØ¿åd¹½üOqAGNbll3FGL J0611.7+2759GB6 J0611+2803?îe®I÷<Y?¡®ßý?w~"ˏ?q'U@Bø
?¦Äë™ 	ü? ›(W£…?ìw$9üY?±Mã§á"5?rFB1c\i?xÌÐüÒæý?»"{;Eât?°˜+0S‡?íÍ¥!.›@?šÙöÆýG?"Ïb÷™œ?Tî2dä?®!ºtœ–?—â .ð>¨?ívº¦7?{í/ö?Ef?Š¶zI?a
j~'N?°ö4³Ož?z$ &Ù6&?ëç°·S¤ÿ?°E¿7D:?"dê‡a¢?šQ?»éuJÀÿ ?­ˆÔ½k?ç¶%<?Áö¼tåÛ?‰ŸˆSȕ`?"‰öö×/?Ñ—ˆrTÜ?ÁŸå¿s.1?ên^âæ?®†ƒfw9e?—éÎRmg
?¨/ \Ÿ?ÃIL,Üàt?«åiÛÄø?ê	N9ì,[?'êc§¿?œ:.Ž®?z¾üÍîýN?ÄSFçp?'Ç]¥Œ<AGN4FGL J0612.5-3138?îÍ4¸æ³JÀ5Œ
9>åïÀ9覨uÕoÀ<5Ûèɂ•@¸ïË)Š@îòžîm1?¶1Õ i"(?­õ}FLÒ?ñÒ±HL@³×1)Þ?Ӭȵæ×:¿äayÝf¢÷¿çéµ²¿èfu 3Ä¿æTg–NÝ¿Ø­>2­AGNfsrqPKS 0610-316?ïøâ¼,'?<Co¥Üj?!WÅkm•?¶8ÎYà?H.¹åo¼¨?9Ã̓kÑ?ïéÉ"Pë^?f:x"°Áð?.Á‰¢™ùy?:øƒfùí»?dJÅOš¼î?dJ}G:?ﶳñ3´b?pÌßÇôFt?V…Õ4)ô4?Z¶îáÄ'?'.håœ?n®Œ±-þÏ?ïÚû '†?Nå;QRÜù?Mç ‹q³?0Yïi§A"?n€B7Œy?K…špÚ`?ïð¬zòºr?Mõ<«d8?2$ܘc?$ëÿŽJ´\?Z'WG?KŠsµƒÏ?︮"…ú?'Âë¢Òß«?E™¬Ì$`?W=å;*?€zÀr™Î?/\¡…
(?ï~c¹ŸÍ?}BwÕÂ?bIþD̵;?^Ó;s@?‹Ô'û=ƒ?{HÕGI߀?Ú2Í?n…Žnör?g6lÙ11?QÏÀS.[?†®0¡ÕË?jÔzˆ·ÀAGN4FGL J0612.5-3934¿³˜äÞì}ûÀ7ùrÿÑÜ×À:ÒȏPj|À<a3œå~t@蜞¶@M¹â}q?Ô%j­¥j?Ã÷‹<^«?ìJtÎ6/@ØCÊZ+Æ¿ã<~֟´f¿èâzžµÍ¿æ+@àðÆ&¿àó"aÌMÌ¿ïÿÃF1=¿åœúÂSw AGNbcuPMN J0612-3939?ïȆâ»T2?v‰<V?Q²"Àáêf?H2È^´$²?wPê`:?uOـ;.?ï̮ޔY?s e"À*??H¡'šcìÆ?Q'[xâ?v"^KÛºÂ?p¶.§Q?ÜIA'?ƒßèUçښ?c–+%̱?lâTstÁÉ?Šj¾ ç(?Éø$"é?ï¡9;"‡?aµ®{êŽT?Q¡èK%?3[¢-9?…'<á"U??`×1×÷ÎÝ?ïb̍^'?"V¡ûjæ?`9ªJˆ»®?Y2á(wa?'ŸG¿u[?'¾øs¥±X?ïZ|PªC?")E4Ñá?`Ó®y8?oâPJýÎ?'–)gú³?'X"ÝŒn?ïáNRã?‹2E›—U?kàúÑùϓ?p$÷æÀæ¨?˜ç¶Ó©Dc?‰*BTÖt€?ïMeIÁü?~È&#pŸ?`q"Ö4)?Rêø™?(0ƒ}
ø?}´FršòAGN4FGL J0612.8+4122¿âWÉ]#@%ÚËB‰ŒÀ7ïßlÁÕÀ;YKHÓ®h@wáú†n?ýQýýûC?" ç^Ñû?»Ù¥ß^[@ ¶ñýÞ½@¤e¹˜<¢¿¾+"˜†I0¿Ó™ä'¡¿Üýüdêæ=¿Þä[^Ëg¿ä	ó‡K¹¿æ°T%òAGNbll3FGL J0612.8+4122B3 0609+413?ïžWðñ‰	?"JMq›û?S1<¸•ü¸?Y'gŒÍ̆?†Ü-'àB?'±ª©•Ü?í¡'Ñ?Àng¸\8¡?› FÃõ?ª¢¿§4?±7‰CHÃ?»'|Ò 8?íµT"³¯"?¥/ËXZ>x?¥Ñ"ô[?žE[Æþ–C?ŸQËU§?˜Ò…'è%Ž?ì9>ï˜Ãu?žæ¦2qQ?œÀk"_fÈ?ƒ6¾*º1?·í»}ñ¨?—ÊÀµõ$?ï'ð(qŽ?‰û}›S†y?Vl"Ù6¸?XA;è1ù?ˆ¯1KözP?ˆQ"'SQ?ê"ƒüº?Çd­'üŸ×?±‹ÊÇ£'ù?¼†–Ý|_?¾o™ZÞ¸?Á¤ð ø™À?îIÖÏÉÆ!?¡â}W&?˜XÏ,¬?™
Ïùy‡?žlVßB—Á?˜*Ÿò°(?èOW3Ìñ?¬/šë Í?©à#3^ã?'4ÖœÕ?ÈJšbÂB?©ó'̬4AGN4FGL J0614.8+6136¿Û
(l¥÷@3Ùb¶®À: èj¸¿À<l³â;ë@35í!Öê@ž7€ŸÍ?Ë<b[ê·n?ÎWÜö:¯S?ûUÕ¤â¢ø@
8Xöh?ïˆ;¾/á¿Úf2CÊF¿éƒ<€8õj¿ç)L?Í¿ä됧'i¿å"ߨò}AGNbcuGB6 J0614+6139?ïèøv–+È?|՗Ì7ð?P€ÚA?e-O§.Ãè?]ý–¾ v?sµeÄ?ïª[™êÞl?"ßõX
0‹?cgªFږÏ?o¯wÝø:Y?€.첇[?}e´Šå?ïN·CVI–?ˆ´Bô8¤÷?{íju©?€±0¶—†c?Ž‹8{ô!??‹?Àˆ'?ï·Óvñ4?\
ó‹–ä@?c9°LÑÑW?AТx®­±?zÖ>ßm=?Z}(ÙÂÆe?ïÛÊgSž?df"R`Ý?Xšd¼¸m?V>ëª]ä?gèf?~âà?Zºi—}?ï÷Wöó"?Ÿ¼PÌÍØÎ?u5bçn¢??"´aφn!?–Ó¼I)¼'?—¡Qp?î¬hMò&N?"ƒõ%X™?³ÉNE»Õ?Œð¢Åeí?›™—(¼g?Šˆe$Ê?îõþìµ~?«ö~uG?
ƒ¶'Wd?e],:™?˜¹|EÈL?}ÒÕ'IÓAGN4FGL J0614.9+2426?Ìԗ±âæ•@§TßÔÀ:‡²Â_‹À;ó
8h&Z@´•‰¿‡?û´Õ)' ?Ø쒅(Ht?怸!D@X`~Åؽ?þ®ÓdìhÉ¿ïü0g¦ØF?ïüÕÞÄF?™óMa[¿Ö'×ÞxÆ»¿ìÛU%ÌB¿ïýCŠUAGNbcuGB6 J0614+2426?à'D-Vz`?ÄXÅe'?°
D·MÁ?¤xÈ ¤p?Úø&¡n>?ÃË9dOµË?ÕÉiË §Ö?ƤàA?ÁžoN8êz?»Z³‡fo?೯F¡qw?Äh…Á[»¤?ãà<$ë¿#?²=‹éO0â?¿‡¼·ÖÆv?¦†=ñ?Ð]˜ˆ2Ð?°-¼¨}?âR²D`W.?¨C¼GQ?º«›òã¼?™p?H¹Y?Ô¯´z½Ø¶?«Ýj*=?ÖSº×	š?"Æ©i"?¾&0Á=ø^?±iàLê?᳊l¼'?Ã:üL¹Žy?ÇoyÛþ?Ã2‡QB'Í?ÇèVb"¦æ?æ l‹][?ä*#ÉG?Æ[J¼ÅKW?ݙ±P‰I.?¶sHbA?Ä{é8?¬È€á­©?Ø(Zi5Æ?µ#¾Â"BÙ?ÙÅ@ëœ_‹?°PPÜX´a?ºS‰Ñ
Û7?§\Ã"çD?ߥܠ é§?´R=•óØæMIXED4FGL J0615.3-3117?íQ®žìó;À4ÛaE•5‡À:Uôÿý²À<hÏ(ǟf@ú¹žßZ@Ò[YÂéõ?½r¬Dìï?¦¦˜ZªEŽ?ç/œÛmy€@Á–vú]T?ïþ?üšE¿æ¡³^f½¤¿ã&Àþb¿áSÅDBO0¿ãÖàµwF¿Ýš_ý–™4AGNbll3FGL J0615.4-3116PKS 0613-312?ïísž»Êú?QÛ<Sþ¼×?1Ž5f¥,î?4Z
9³f?`Zšb¼Â¤?PK³‡BÏ?ïÞ9ãä¡?l©ê&Q\?8v<4˜?A‹Øà/@ç?n·DƟ´U?jVI"E?ï®E@ãZ?qrÙ®×ù?U‡1ë7?TŒœgˇ{?Î~á;?pm*·Kù®?ï°fc–?]—Ãa±NV?WWüN[3?36£ŽÅr?€ûgÄÿ0Ê?\¡Ìž²?ï×úòòGÓ?dfµpٔ®?Fntæž?BX¸æÐm?q@8½&_½?b4zŽò
Ç?女f|¬?'êùÖÊ?KýB/&P?["õ®±ny?"ŸÒZ尝?îo><m?ïpI/¸™(?€DrùWQn?`u¶¢SP"?RÃr^€ä£?ÐFm¼_Ü?~$-{Í"?ï
æx­?y5œâ?pxb?Sž°Ñùm?™ Zýc?yƒ;À<ÉôAGN4FGL J0616.1-1732?Ø0eäÀ/j;Ýü À;~ì\µ½À< Òc傦@!÷ŽsuÃ|?öښéœ?åö\å®›?Ù¨Ã"ð?÷†D·%?þўEzÞn¿ïþ'!€-b?ïôJõǗÚ?Ñú±AV¥¿Ø2ÒûÄ¿ÛÓmE'ÒW¿Ü  0÷ïAGNbll1RXS J061609.5-173313?ï²Dùâ¸$?†ÁdM?M¡ø"ÀV?UIÛS=ã½?"¡óêL×?ƒÊ[Çf²m?ï¦@Çy€?‰¦tÞ??W¨ÞÜEòó?d"6ü"T?ƒz²=÷QÇ?‡¿]Öþ\š?îº)Ît[‹?–°ýWj?q¦!°àxG?vËmÐÈ?¢(žá€XÃ?•SšnÇ?í¾_[¸?‰Þü,êLm?fùñ}Æ&X?X²Üï®Eó?±U7¡aL?‰¢$.gÚJ?ï•%r¤Ï?'rá7'µ'?Y—¿ƒqè?R¯â ¼€?‡"°x7²?†ê;é¦?îÿmži3?¢èöø:%û?qC(w,,:?'@ûYei—?›Á'—?¡Ä…ÂêN?î7+ÌrÆ?›Ñ‰H?u­Þ@Ÿ0?y+"<?o?«fÑ|Q7À?›(SÐ.?ë"=Ñêu?¦?çhÝΣ?_]Çėϋ?cs5@yxÚ?ÁtM(kÍ?¦RtÿÍAGN4FGL J0616.7-1049?ÛeÑ£À)"Í[h£À:N.a<[À;¢ûú·Á£@G˯ÁN>@ãÖáù"¼?ÐÄR1ž‰?Ù¦žD¤Ù@ñ©áyñ@—rÄÔ?ïÿéà
v¿è@‡å</[¿ìcMâáâ¿èá}ÿ	_û¿ïÿÿ" 5•?ïù*ù¨ÍêAGNbcuPMN J0616-1040?îKú
'|Ù?®)¢ã/¿Õ?Šê‹6šêÔ?£Á¶û˜!?¤…¼[Õ,±?¥)ƒsFÜy?ì¸cÛéí'?¿(‰¿€?–:0ì?›óàxUp-?´»›TJS7?»M'P&'?èˆÁ:ü?­æ`–Ÿ'x?°¨\ù̓? .ݧÕ5?Ç¡Ÿú~-O?«Ks'"…?ê½(Â'i?¡;û½tA?¢—õÆêUa?ƒ3J¬òž?ÀeboáºE?ž#â»Õ?ìèÊ	Vž{?·§ñsþ³?— 
Éc®?¢S¦Ó
uò?²Ñ¬Bò ¢?³À Ì/?èc+ìËxm?ÊDÇxW³#?·­ÛQC?¾>ýp{
?œb£Û‰K?ÄñQ™`ö?äÀœ¤Àn?±ÆàÊf³A?º[Œ¶ºÅA?¥,þ–Â{o?ÏÏÇ£›¦?­³õç'Šì?ᓹOŽÕé?³£5ƒ'?¸¶âÖ§Ê? K`÷G¼Û?ÖªÔ«y§?²c°"þ¾AGN4FGL J0616.9+4340?íuôØüÓG@)<ù;À oÀ;ÚÂXՄÀ<À­°i@"—¤}£Cç?ù¼'«A?Ø	zg¥*Ç?¼O ÒÀ?éÙ? ý&?÷Š¿Ì‰0¿ä¿@OÁß?ï«ù4㍿ٸ)|¦Ù¿Ý&c–þ4?"™húÈç¿ÜºÉ?$AGNbcuGB6 J0617+4340?ïp£cm?ˆ× —î?<ݧj1Ù?1'µÕÍà`?'x¡e:Î?ˆš×¦'n?ì?ØÂMy?Á'˚ŒwŒ?}«ûÚvš?†¼Œå`b?¼&z4›àh?À'¡Qb·õ?î£Ï
Õ?'!a¼—ý6?lNBÕՔ?p3ãLå¿?£þ+8™Í½?}9=?îk–²Å Å?Œ?cxc?hχ{Ú¢ì?YኢÝ?§¹œ_ÅÙ?Œq¬
ç(¬?îÃá©.?	ÿûá(?KŸ+»ê?C$"wz'ã?£Sq½Ã«¢?œÌ+ Æó:?é
Øwzá?É¿p|ى8?‰e>?³?šðûƒ®¼?ÊA º±R"?Éc泗‹f?ílÇØò?ž7wߌLg?wRžt"?vÙ?Í?³$¦^–;Ö?œôuêãš?ëŒJ€y.Œ?¦(,¥2?taß.ÖW'?v6¶‹üÆ?Á+Ç4<ó?¦–H>M½AGN4FGL J0617.2+5701?î*
ÍäNõ@2ëáe
FÀ9I"žˆÀ<(ØåßÃJ@‹AÑ܁ @a´5&Rz?¦DpÈ??§_™m¤É#@"'Æ@
Ð-µý­¿Ñ£ˆ{>1¿áZºÌH¦¿âA¬=
LŠ¿Ü"ëø>ø¿åø| µ¿ã^'/éAGNbll3FGL J0617.2+570187GB 061258.1+570222?ïõñ–'@®?FÏÀm;€?/þ}a–?#|}p.ܾ?P‹`/?CSu_:Èe?ïÉJsŽ˜?w Õ~?TB¿îV?`¿" þ¬?vJ'ul?r÷Dh¼aX?ïÈã½Ãß,?`þ¡I¨øØ?R§xi)?SôŒCž?w
·'8óû?X·-'Ó8Œ?ïÃ̟š(z?X4x
rü?e̓šk‰?FÌ­¾ò?s2îÓ'?Q¹Íþeu?ïí>¾N&?S߯""d?@-P"/¤?3^6Ƶ>?]Äڀ妷?P]÷ô~¸A?ïnSᏸ«?'$ž¶] w?høçk¯?xti7<ßZ?Ž-^¾Þ??‹
R@?ï§5—ð?qZ+ŽÞÞ}?Z…hj¼¨?Z"•™	r?'í^ÈL\g?nÓvò<(h?ïsì-\¦ì?ulŸSå{?z¨!§±"˜?eƒµô¿•?…°ã˝*?l¤©²‰\7AGN4FGL J0617.7-1715?ÐíÊ›¢¼À.!6ŎêêÀ9"#rËÏwÀ;Û¢4rÎT@‹-á
¡?üœ¡ž¥r?¶¢?/•ÄÎ?¼ÜÎ!¶‰@¹ÍÄC'O@v]ÃՂS?ïã3@Ÿ-¿àÅã~ê읿ÝÈ輗u}¿ÖÞ$Þ[À¿ÜàA>
ׯ¿ç=ý¼ƒÔAGNbll3FGL J0617.6-1717IVS B0615-172?ïƁ½˜ó?oÂƚ£™?N×êA–o?CM†}0TÖ?xä>³5ù>?lÈÚ݃>¾?ï®dòìº?Œ4<±Ùy?YÏ¿iæH?_W=A¿"?,ËhˆO{?‰¯dfnå_?ï0¨ý˜OJ?†±Þ•ê;?pÓñaà"s?l——'в?•µãô~?"(ßU¼#J?í8³?‡›4óS~•?ƒ@ o¡Ïy?^"}YŸ¿?µ?+¸Ç[?†šñdZ]?ï‰à(Ÿ0‡?|q!òÃR?ef¬ó˜²w?Y'æ›L&?ˆ.J›M±‹?y
ðˆ6šo?ï	Óøÿ? ¿'²-?w¹`»Ùï?Œ'jø²³æ?™í®!n˜?™iJ5G#o?î[ܨ?­H?–â^VҔ?'#ã¸`T
?~æ!VËE?¥¹<Š‡?"–¦žZ‹¡?é2݃1? /wKº?" óåq\¯?zJüE:è£?È kvVړ? 
þ—™;AGN4FGL J0618.1-2428?ê"#ÝøÀ1՟+©ÑöÀ:Žîr9€À<Q·åž@ñü"up@ÅsS6?ÊvófêoË?Ê\o—'ƒP?ûëlË@5'éþâ¿çzŠªéM6¿Á™Ãàêç¿åÈÜä.¿ã"I,«¿íÁÍÊùö¿ï‹›ÿûMiAGNfsrq3FGL J0618.2-2429PMN J0618-2426?îß+ž‹¾1?' PÇ})?}k1Œuî?rZð¡ž7?œ¿¿Ïâvš?ŽJúi§¡?ï~IRj—4?‹=¨ì˜¦?mdÅ8‡õ?p›Vö
‹?‰£øƒ
?†¼Kˆ¥½?îÊ"ú%K?°Ïj&‰?"wÃɞ‡?€\?úi?œƒmÚºPg?‹Áû®#ÎÃ?î]S,DN?|º'íÇ?Œmv#h|ü?hN)î5ß'?£oµtµl?yåyJ¨r‹?íäV´Ë,?¥—r7ô?•¢8÷Ûq?Œ@+÷Òw?²€O
tÖÃ?¡ÐTpä|h?î–2qõÄE?¤~'Ù7	?…]]V±ã?'~ô£®Û?¡Y‹Ý.?žªùÃnâÞ?í–G֔‡ó?Ÿ³Ó¶åŸ?"ƒîµËkˆ?‹xFïšÛx?¬Y‹:õä?™¯*5ÄÄ?ìúUP?—.îÝ3?žâbâ؏¿?"}l¾Q?··'Å«J?"÷ÊHAGN4FGL J0618.9-1138?ï»Ê0@ªÀ(Ӝ"öœªÀ:%'ºZ'À;±B¾ÁqO@¸w¿T>F@	1)Ì?Ïåwh—C(?ӊ©|:¹@W
"˜±<@
¯î~Î<¿ÞUµßJ}Ó¿Ù@½!Þø¿åÒ!ÀšŠ¿ëò9Wÿ›¿âÔrþ¥7¿ïÿ­AGNbcu3FGL J0618.9-1138TXS 0616-116?ïÕØѵ6?r웮£•<??'Lø?5¤i¥¹Ï ?s|î¸6í?r4Շùä~?ïm²à^òK?""€Rñv?coÀgƱ?k}
!)
?Ìì—×t?'Éåî…$?ì2îò¼u'?¤€ø°LÛÈ?'®ƒl£Å¬?töˆCA?¹üçÏI?¢ÐY\-K"?îyq)§²ü?~‰3[Sâ?p/&Â5;ð?R²yւóƒ?¦cˆÆªÍ?},˜0+J•?ï¦Ü»WYƒ?€Ë·ÕÃE?M°ïF:?F€•rµ­‹?"mÂ,ãn?€4
¢ü«ú?îdç0–?­',Ä­d??†D(ªÂV"?™oº¡í?¤ ƒÿºœ?§'ËNõ?êeó¬ÏE?®—Æ"7?–Ãrs?!?Íü(®?±?ÓQð§aG?¬c'^Ô­?ëÝºA/?™ï'e€ªŽ?"×­«"Nù?rE—زá?À{<|"?™Fú¦©ì[AGN4FGL J0620.3+3804?ì¾Ïµ¤+@%|L7æ÷À:5ÉæhÀ;™4A@3X¡¬¸…@#ŒÚnuÿ?ÎP¹ŠÖ³?'£7'3 –?Ñî¼t@`­Eîé?ì8npöã!?Û{ļ²ù<¿éÓ¯ºmO¿æ(ýð[GN¿äêîU³¼¿ïÿöZdÐdAGNbcuGB6 J0620+3806?á[P–£ùx?É8œ"NÎ3?"%uf{¸?}P–~…º?ܨ}¦ãã?É<M¹j?ér«)þšê?Æ&
֝±?™þVY>dß?Ÿ^ð§dD?Æõˆ'´ü?Äs|YAå©?௫{L?³¿•IÜ~?¯s/]­? ‰ï9€¡?Ú²C³©C?³¸å&o\X?㯑à荞?ªÙæÄMTû?— '­ý¨?z«ÏÖDË?×.Ôøj?ªþaƒùU?áG~ùҋË?ņ
d†V5?'пªã3?Šš'dÙ$r?ÜSöQ¢p?ň½ôlÎà?âàŒ²«cq?϶@N#Ïh?­EˆóŸ˜Ž?¶XÑðé…Â?֖5{âÏn?Íñ5¯0Ñü?ÜÐÌÂw£?´[ìs]?±âÙóÌ¡÷? •i9Åk?Þ¶|Àè4?´æ_÷G°Õ?ÕPY'þ:?±w-^T?£Y·m"/?Ž<¡Á½Am?ä"7úå†O?±FCoç$¯MIXED4FGL J0620.5-2512?î}2•Ôh"À1™ºç£À9¬6KìgÀ;å &5@añµaÌ@]d_%)…?·ÈG¾àù?Ï°%1½½@WƒPù@KF?jú?·J@€x¶J¿ã*óÿ@½_¿èYö|É¿èæ	ITݨ¿ïÿé{2¦¿ÓÀâÞ±ü'AGNbcuPKS 0618-252?ï¹ÍÍíx?­Á/
HbÑ?n°ÓU}º?z¢~UÒº?tÀÀ•€?­‰ìá·?ïԅÓ5"?v‹MøB³º?N¿xa¡ÁÂ?XŒµ‰Oü˜?qå'i'ð5?s)-ª?îÍõE*ÆA?•­÷ë ¯T?"îg<ªI?'ÿ
"€°?'³hõ"["?‡"1êk•¼?ø}:ú?j¥µÛ;sø?q/èçéÀo?U^A´ÂH?†ÅMk\‰2?eÐñ?_ö½?ï–ÛððÝ<?£Ô;U;|Ë?€ìâ/wI]?ŠÕÙz€å?r¸C5³Y?¢t—Ö á?ï_±xTòÃ?—CQŽnì?s
‡óß?‡Ç‡bkw?Ž
ïÆ?'7žݧ?íÓú@ñ?¡is_hÞJ?¢}ç˜?™ßnSßi÷? @à$Ue[?""Pð¬}?îI3x†??@?Ú7N?¸Y:hb"?z¸}9°‰?£›ÙÓÈ?‡ûŽ$r/…AGN4FGL J0620.7+2643¿í¥ÄF˜–@¯^AÔ¶¦À:¡…}'ãÀ<E-5Ã0l@#XÅq8Ò?ø‰{>d¿?ÀÜ gS¡=?¯pÐDÅ?ñ&'+½óì@<HQRƒ¿ïø½Ÿ¤v¿î¿ >ybm?ïÿ!ž5_³?xõá)a^{¿à
Ç9G¿œô"'|êAGNbcu3FGL J0620.4+2644RX J0620.6+2644?îc¥Ï?¨F‡É»Ä?PÙJc•?A¹¥yH?©D¯Dl9¼?¨(Ði"?êuRæ½õÖ?Á§
Â¿?p¿¿mX;?€	égþ8?Ť»ÖÛCˆ?ÁO.©9¸?츟¾C>'?¢RCBdÌ?g[÷Ëqº?bÕð†;?¹'o-Áo?¢'åY-O?í¢)Û¾?'ªŸç–››?]Û9b'?Os¡påÄE?²t‹NDŠ?'°C¾Á}V?ìã"['Bª?±Ü¤a¯Ùˆ?_.Áæí?RïYu¯]?¸gÜf«';?±¼«ªÆÆ+?äÇÙûß^ö?ÉhTóLhc?|ßp| ù?ŽßèŠ!êQ?ÕüÎF8ba?ÈȔvøy?é,IOìQ?¬™>w†‹?tús J²?jTÍ´>»œ?ʧe[	Í?¬‰†["?éÀBò‡¶1?«]x¨žŸ\?roW¾ePq?qÔ.î8ƒ?ÈkywÝ~˜?«t1	 -VAGN4FGL J0621.2-4648¿îis¿}fÀ8]æ?À:×Fšï/À<{«?´Jö@€Ñ¯	ÃM@Ò>ƒÉM¼?Êõ°kϲ?ÀôºQ Ä?ïü"à՘M@Éf'0CÀ?ïԉ>؂ã¿å©é]|2¿ç)y
­Øì¿ë);b¬'¿ïÿ¾ú¿±€
A/šAGNbcuIVS B0619-468?ïÎï(Ž¶ß?‰§E#¬Ÿ´?býʐCnê?‰¸}E·+?n
?ÁÝ?iw3"*i¶?ïfÁ~ƒ>?Š_à,‹?pÃy¥Õ?r"<`RI?Žºï:ò?"¯ÕxËvi?ïRºxk?€&‡9€æV?q×w!~è¯?p/Ø57ѝ?'2Ó:Dâm?{z®â™?ï'ÐÚߛB?rVW—ÄìÔ?{ÂüÐ	À?[ä#ۛT?"\Þ}N_?n0Ä&ãª?ï¨ÇK¥è)?yÃR%Â×]?Z$½??Wâ_¹þ?'‹Š5A6?wÈ'(ì?îUÕû´?¤ÔÕ›ŽY?'»t4ƒ3?êô-£w?¥óÑ3éÛ^? :v·oÈ?îÈ:UU5Ö?‹*<i'À·?z'î Û?u÷ ónŽá? +üØ	?:?‡Ìeù´*?íT2M@`Ô?'d&Ո±`?"Ôe¾û?}!n`¿?°—ø{±?Ždñ#÷´‹AGN4FGL J0621.2-2213¿éãÀ¢-MÀ0LY§;BÌÀ:¸
!Áñ§À<vžy_g@"SCôÌp@b5deÛ&?Í/ÉÜ­j‡?Ï'쮤@=–é»ðÜ@Æi'wâ?íÌÙ,V  ¿äˍ Îí¿ã§".οâ.0y²É¿í*áã¿ïº«ÍxÄ7AGNbcuPMN J0621-2213?ïlÀ·YŒÓ?³YÀøs¾?gür¤.À?Š"jûË?	"Ò÷ˆ?±ssÙÛB?ï˜ÆDaw?"iKÚ/G'?eî'Ûñ–"?k<`U¶??"Rʌ²~¹?IeÌÒôâ?ïp	êÜϜ?€ã,#Ž>`?sj9aMm?tä¼×Þ
#?ŠHh›í(Y?x²¬–õ›?îïd+[?räYõ¬wg?{ê;ïV¦á?X_ÉÔä?›àßnß?pýÑ¿â@ð?îð¼­3Ä?¬zMiŽe¾?wÚ¬)ƒL÷?€ëÈÙ¬½æ?›ñ¿G"ü?¨ƒûƒ¶±Â?îÛÌ@Ø.Í? ½ÿ™AžË?y"˜ÛúW?ƒÌrŠ?ž%Qª3ô
?œàË
XN?î÷™@G1²?èíK1?!2«MŸ?|¼®D•?™D"eŸ'l?‡°ÞÛI?í
Kò¿,?¢¹:;¡?: eº¿»?uj‹^úSœ?³‡R¾0*?Ž•8xüÇåAGN4FGL J0621.7-3411¿ï°,ù2[rÀ4"D€bïÀ;ö¤À<‹S+ ?;@ L'Þœ?þZ˜⚔?ЙÇ|Uæç?Äx†$?òbI$.?ÿ‰®ww/â¿àÈA§õÓ¿î1­ÂEŠN?¹ú[?/¯Š¿Ýkq}›·+¿ãQf™'
¿âõÚã1AGNbll1RXS J062150.0-341140?ïÄáyHª?q©™óÏ ?BNÍ^V¶­?4,?	ó)#?{EiÀ‡ÊÝ?q ^&?ï'ó<®?†Pãâ?c2'uú2U?iWeÊ@Õ?†vŒNW{è?'[‰cx?ïVon*ˆ?'•"JΟ?aQ[ 'âÂ?`n+fì	\?"æÏ
Œ?éR€1¾ì?îô8ª*?Ké1à·?h²üö¥T?N/k™Þ-?¬õ'"Àç'?5™MÇ»?ï'(•4ý?€ùgÀo¥Œ?Rœ'8Ç?DW9îî¹	?‰bhíä¦\?€lÁ'Ÿ£?îìàϟKF?žàQE	Lï?rP]}AÙ?èÆ3#ï?ÏάB`?›§å'Z¹"?îÝoyàk»?ŒÓ¦BºÞº?iÓG¹?ié/PÖ? ˜°hý•N?‹œ~Lø[?ê×6) ¤?ž…0ÓrÞc?vëäÂpS(?g•pqL«?ÃëÈ4%L?ž!
Öa×AGN4FGL J0621.8+1746?á¢gÆ/F6?ûyŒ³Ø	AÀ:¬¬ÊÎÅËÀ<Û£)eT@!å°²9ùv?ýË?.9?Ìa2µ^ñþ?­Í bSºÆ?áxg_µ0@<¹y]å?¶ÁŒ@¯aq¿ïÿ…ãp?ïáeáhö¿áQÛm¿ÐÄށU*)¿Ù\+d‡¾üAGNbllRX J0621.7+1747?靺œã>î?Ɨä1\2J?WåÐÚóˆþ?Jþif §9?ÉYI꧶?ƚ¢Sã"?áÒÙÈ?ÓXž@Œ&?vÔY"8Ýå?…`<ük¾?Ûþûۂ?Ó5Ç£©N?냯à¶lA?¦T
¿Ý·<?twÃ	Vú?s6ºÄeé?ÁMˆ AáC?¦;&ÏPv?î+j¯vO¾?ŒOtfÂi?HJþˆ¬8²??,ªO²#Ó?¬è)
ð†×?Œ#,sßq?⷇=Ó?Æ<²
Ý1R?g^üìÐzc?[›*úáz?Úb3‹ó"¶?Æ9¯_dР?ÚwãïÜ¥?Ñt;?Šô)?qÐøýî‡ü?ƒÒ4^º1?âÏ¢J
•?Ñk"¯ð?æ®v±ž?²èÎ	Ë¡M?7Î:šŒ‡?wëk×h)?ÓX810	ï?²Õ—²ÊÔ5?ëNÙ2qþ[?§—æî~Q?Uzíb•µ­?Sœàöx`p?™¥\_@F?§"–êG
MIXED4FGL J0622.3-2605?ÎÐ53_öÀ1ŽPÅë1<À8w¬-ðÔÀ;¢ªùš‹@ûNuÙËä?ý÷dñ`¯?¢¡È€üƒŽ?
YJI$a?úbxÐÌ5Î@8xé@¿á䥜[d¿ØqCå+B¿Þåe_€C1¿ÝÔY¨‡s¿ÚðÁ^.´s¿Þìþ¢˜œAGNbll3FGL J0622.4-2606PMN J0622-2605?ïùéY(?8ÔË÷˜~8?›è,Ãà?ðOX·?IÀ'û'$?7¡Ï6Äcp?ïîÚù,Ʉ?eŊp"?*%­ÄœÌ?7bšû½6?_Wàî-?cëZç58†?ï–ö:´ÿ?"¾è$â¦?V'@ɏN¿?^6Áú‹?‡}‰^1:j?ƒ½Æˇ!¥?ïÞjgŽç?P܉‰Ó<K?/µ¨(yƒ?²72v,û?oš>%ó¹/?P=v'HJ?ïój¾9áù?IŠ¶Ø]¶? °(D~$G?™E;¥Lô?W~T«;J?H@˜§¦T—?ïÒämà?~ËÁæfL?@øÐ7TU€?U'{5Õù?tnÙ¬ûq?}4ÔÔö?w?ï`~•¶?ŠÍ=^PŠ?a4)·»@ÿ?l%s»RÃ?'É·zX€?‰·¼¬¶?ï¹³à—¯à?i NÇQÓ?@x!¹—"?0ÜføÑp?€‹…¼»ZP?h8­aʺÂAGN4FGL J0622.4-6433¿ãp»Ô×ÞÀ;bÎ-±êÀ:»ƒÑÀ<W0º²îÕ@zô»Ô,@¢¶®}Vm?ŝßN"¿°ÊkÞöE?å"Èy€õ^@'~øƒ‰ã¿å@¯½ÈM¿æäÚ_²m%¿îA¨v¬.È¿ÒÊrŸ¯³6¿ÐgÕÒ/¿ïýßßy!ÕAGNfsrqRX J062308.0-643619?_ß[?Ž‹~´ø?^$ÞÃ,­Ž?_•/'ɦV?†ŒŒ)"Z?2Ñ^©o?ﴓF)–8?…Öû5&8µ?Te—(ç?bSÆúÙª?€N{ÿqì?ƒ¤îöé?í[MºÒÇ?¢–Û_rèf?uÕWëcb¾?|n¾DA£?³ÈA"§?¢7$p¬ù8?ïßDwdv³?YØÔ;?<I0^æ?
?16™5?m2b²¸ˆ¢?X>BÖ Rt?ï|Ž€óŸ?"/ð‡?p^y9R35?wGºÄ)—«?ˆ­ûŠÚ¢?8‰ú¹Eç?îå€:«€*?°×g9ÝâÃ?l3;Ì áC?~Ú
&€³?ŸÉ'6§9ž?°!sÝNMŒ?ì…Ø©úºÇ?¤ÿ'ýoä?{ò{Õç>?}™?g++?ºôpÍ?£•¼äN(?ï‰A"Æ9Ç?~̙{¬
?b¹à76?cÙ	un1?‰o–»Ã»?{Ü·8ÙjáAGN4FGL J0622.7-4141¿Ð…3ÇløÀ6¸¼M"ÉÀ;Ć­-ËÀ<ØmSÀqu@œêxÚ1d?ÿ¤2‹m‡?ÈeŸA#`Ø?ÛKkä)µ±@g ã¥Vf@ãNòï¿ïÿûÎBÓ?ïÿÌÐJ†¿ÝÌË_ºOÈ¿âqß«Ì¢¿ëäò}¶d+¿ïÿå]½JyAGNbcu3FGL J0623.1-4143SUMSS J062242-414357?æ\ìF(?ÃyƼ"Á²?ÇÓ4£~Rt?ÀµtÉM?½r4‡¾r8?¶hÆî?íœ9©ïÓ?«QÚ͝U‡?¢;íw)f³?¥9ãUÄ:?¤wåå'?˜&ÖÄÍmê?æKHtF"?²,ÁÑõjK?Ç7Y?­IìM¿¨+?¿—Ž*êS4?¨!|§K¾?íCäù¿I,?‰áZÛ/ö?©"È|?ƒš 'ò¼?¢¯ŽR²-?ç¯Xí?嘷5O²?Ã6g>ÂLZ?ÍYE pÝ?Ârz}Áï?½°tf¸?³ÅúÝ)±í?éSêÁæ{?Âc$ûÀˆÏ?¼µÿ‰k+Ñ?À5!eçv­?¸ªªiô±?¯Ð© +`Ú?á—ŝÈA<?¹tWÃö?ÒG™ƒì€"?¶Ñ/_£…?Ŷƒ+»g?­Ð®à{öÞ?éªÑå»[5?¢Ó
3͜\?»7ò—"

?¤ìK&ËÅ?·q~=¢ÁÄ?–Õ-&PbAGN4FGL J0622.9+3326¿ä¦Á}¨@"MŸ±áŽüÀ8k"ÌÐÿÀ;fr° Ĝ@VfXN ¢@D:Âs­? §?ä5bý?´8p)³®@KïIÏVë@azXᘌ¿ÑI
`EË¿Úölmçd(¿äÿ­õœ¿áWÂ~ë'¿éB=äg¿ã¶ô›»³AGNBCU3FGL J0622.9+3326B2 0619+33?ïnYÊv±7?€ßœ¶ñ"?^ÊÇÕeNn?Q™EÓH8?H6g9-?€si¤tl?ïÅ6Ò
_'?ŠTyDˆœÑ??ŸËÛÑ2?O­Ž©t?{jš=Y'ø?‰¥ÂÄK¤?ïa	ûÆ#?Šírx‡??uY_êæ±,?€+ÿÊ¿n"?
M›iR?"ÕÏ£îf?ïú=71ß:?0éôÎε7?>àÉú>÷׃®KÓç?E§A[ÔF?0A›·ýùÅ?îÐÅ4?"œXÇ´z?a¨SÞïä?Xlí{²j®?¡Ù'~=*?"#Ç|Î);?ï'VšÒì?—ILS€?WÚ9Uaà^?pæ]zD]?Œo/Îÿ?–ƒ€VRÀ?ï%È*j|?•«Xm[Kv?×V|·T?‡"@VkÎY?–/¸ToÃÝ?Ôj+ìÆ?ïò5Ñaö¯?N¹U˜Šó
?Œ©½c?Šæás?Yû"!xŸ?M´þˑ‡AGN4FGL J0623.0-3010?ã÷ԑ"ÛÀ2ëèPïÝÀ:Žf5¾þ®À<WoŠÑ€@sªZ1#ä@üCbU_®?Çy-¾T9?È´͆†?ÿ4i^hk#@	—49˜}¿ï©\ºëù¹?ïþ•œ´×
¿çýŠ¥
$¿æÜþ]¾w¿ë>ÝöÀ¼¿ïÿå(
eCAGNbcuPMN J0623-3010?ï×xþª¦˜?lHáÀVÌ/?S'Š›'F?L;ûmQ?nó;É÷.Ç?iVd	BµŽ?ïáà"±øX?pºØláÕF??|®òl?H¼ZŒÃ¢ß?j/ø[ý?m ñfZ&?ï¥AX?'O:u¨À×?töÔÿg|?z˜ª‹ÐGq?—'Rè ?¹‡½Òr¤?ï¹UAc?W.°ì]"?cƍùv7?Dà`B›V‡?yqù^$ŸY?S˜äë5j?ï·B«?x|`ë~›î?bp…ì™?\·Aŧ$?{]ræj?t¯-pvê?﨏êî:?‹!‹|0¹?Xæø{^ž?quDPk5?'¿]4 á|?‡úþÌ>ց?îæXgLb?'NY䩶"?yz"•Ð[(?|ÁZˆÎ¤u?œÖ[̉þ?Ž·™i0
Ù?ïWEãZÊ?u{Ɵâ?vVHˆBZ?aslpƒ>?c=»B#?qt½(štAGN4FGL J0623.2+3044?ï`ÕðYfE@ ¨½#žÀ9Ù©-‹TÀ<E¢Ë@ ¾!Š?üS€*\ÊÜ?Àµs>æð?Ä=ʗ"Z@'üÕ©@&ïjÜlÓ¿âDrØ
¿æBw©"É(¿àø]©ÿBk¿Îêq"'¿Ý`QyoW§¿ç®Žd•AGNbll3FGL J0623.3+3043GB6 J0623+3045?ï±GÔsp?s—œ£i?Xxܲ‹i"?W݊9Uú?€Ÿ#» Ç?pûéôU?ìçÅ®lÜÅ?·¦g;Ü ¾?e:32¢?k¸+ýE`?¸ñ¥Eá?·7"Ìî???îðÕOÓ'?ˆ¬0]µ?nmþ8¿4?f…3퀔?ž–6È	?‡;üväâ?în'š þ?€ÂÛuqÈ ?vEueìȳ?X,"ÒÅ=A?¦VX)ÌR
?€f–ìÑß
?ïV)üÂw£?‡§þQÎ*¥?q¸—Lii?n0_¯ðŒ?Ìš–Òf€?ƒ€Ù«ÃÂ×?èfµå^Í?Æáce]°h?uöc¶ö?€Œˆi9<?͵w»ÎLÕ?Ɩoÿ¨}s?íAže±4Á?žÔÚT£/?'ˤË%S´?|¹D®ª}»?³™˜8Ë?›ÁX¹ûDø?ëáÆýà–?›1‡{MÂð?‹þw'ÿ8¿?v0¨÷ªü?½r֌û7?šmB¸1@\AGN4FGL J0623.7-3348¿íÈô&Ç®ÅÀ4[À6ãÀ9ìuk¼ç|À< 9€
@ Z¬Hóº@bê¾O[ˆ?¶Ô? Á†?ÆÌV»£…@ºk
F@ëc`w?ïeáÜ(Š¿Öæ€',À¿ääµ Þ¿ã²æ!1¨ï¿ë"Ÿ»Ì¿ïù)ÍAGNbcuPMN J0623-3350?ïÂò2âÖO?p¹œ±¸‡Ž?n"2²2?gfd«Ø¹?n‰šàûß³?^qw£¼én?ïç{PD?k—Ÿ	Ã<É?9!Ž…E)Ø?EÞX a¤'?e`Åä
Œ?h9C>€Zº?ïF죁Ð?"5•I€'?næ£É¯r?ŒÃÃs<–?ÿ^%—l­?‡†Ñª|÷À?ïºo©ŸåÓ?]"³ÅË?T[ü'Þ?9;
½ì?}ÂT?q«Ñ?Z͘Xá¡?AÞ?€›¨¨Í?jJ8Ú
?vÐÐÏ®â?zÀ•B-2N?pTä{·ý?ï±Å֟š¡?"<¤÷Æ?V948E³•?pþÖæP^l?€ÇcÊáUg?y˜ò#¤B?îG,ܤ? ;Çÿ¤µ? ˆP¨ÜO?—èÔØCZ?œUϋ<?'67®ôÈà?ï4ñú·I`?|îf8Ü¶?mÁ´lŽ­?ZŠAÅAÈ?•©Š<á9?yðDÐËSAGN4FGL J0623.9-5259¿æ¬ïH'ƒÀ9[ѼrâÀ:è	¬Q,BÀ<£O•i‰1@yfÞ±PÅ@Á¶ža?Àd鎤s¿ ©Ü1ï'H?ãæ¹Ù«@K^ù	¿ê''Ò¬á?…pU0ð¿ä&½2%¿äO%‡N"¿Ò3f~¿á> AiõAGNbllMS 06225-5256?ïÄÔ·8!@?q$!i|†f?H¾L³?6îxCœ=D?z}Ú̖Ó`?pz˜‡SÑx?↑"äí'?•2D‰fƒ?K	JxqM?SNð¦5QM?|ÉÅB¬-^?|øZéOá?ïbq¾M?'@ãÂŸ?cšI^m›?k2"Vz?'LH—™ES?€ÅhE^çì?ïŽö«¡±?h"%Åà•?R¬V–¬Ø¥?:yüwâž?‰ìÊFŸFŽ?h$'‰?ïtnY`*?†ëL­_?]ã¿
¢t?Q9'P‡ÈZ?@¬Š»nü?"úZ«p|W?ïD7²žÎ7?'áÌ\ï­?Y™.©Òr?c½Œª.#?•çPoxü?'¾g¶ú?îìe7"'7?‹!/×\hy?i­õ"<ÿ?fG‹/£2?Ÿ=¶]¹]s?ŠùíŒøÜ?dæÖÜ?…ÅA­·¨?jӁ'&á©?]سü—x×?¤z±˜†!¬?…ÂäpÌS¨AGN4FGL J0624.2-2943?ÓÁyñnÔÀ2ƒ`¦3À;-Á>#Q>À<šnkîe¤@ g
Tý2p@2fâ(r?Æÿù_|è3?'îƒx<t?¸paö"@íW<ý·P¿Ô5k×ÌÛ¿ïÕrùà0?ëFúû´@å¿ãÚ­Ëų¿ê&ÏAò×?ÌJry\ãAGNbcu1RXS J062422.3-294449?Fñ+?‡*ö;)N?X?¿
$ò­?W:ES¾?ŠÐDí?†TÏ羨?ﶮ
«?ƒXeٍúN?TÀô8`î|?`-×|ôµY?x¼Z|î?€½ÚÙçOÍ?ïZxzÒ?)6u¬Y?p'µÊÔ±?vŠ™hÊ®_?›q̅†š?ª†ñœ?ï/}³øÒ?xàD‹š?[<ðÖ'M§?R€Bn†8È?˜\~úê"ó?w¬XW'?îæ^ˆrS?—K󀴩?oÕpg´?xڄ;Ֆd?Ÿ9€ò\=?•îU¿—]"?ïAyäêÈ-?–Ò`ùͅ?cHooÎhß?sTJ{ÂwÃ?•gµy|¡D?"©Æ¨êq-?î;^4‹q?™%Û׸«?t<í×B?|"ÎBäó1?©Â™òHÌ?—ЪÃYÿ?íÌoãÎØ&?–h¤G~Œ?k2¬O©¶r?itr_£?°ÂëBêÜ?•àYÚWsAGN4FGL J0625.3+4439?ﹺDm¡@,Èdìé¢ÆÀ9p-ô/fÀ<-ëÎð"{@+'þKË@j0¥º9L?®Š°av|?©|ýÇ%C?úÔ:I§é¾@
8
û1¿Þi"$a¿ÛQìüíüÈ¿áÖ¸ÞÙ>Ë¿á&ƒÝo²@¿â¿Ð/WÜ`¿ãºû~ÿ—AGNbll3FGL J0625.2+4440GB6 J0625+4440?ïò¡P$ä?I%gƒV?+RáH•÷?Bߍ¬?Xnabh¦m?Gv€}";?ï×~|»E?t'ö$›~?Kã7¶B)?Xýj ʘÈ?pÄZ¯ÆN%?p}öÕw?ï½Æ&Xô?i"Ãi??Ušß«%üø?V_=\"Æð?{¶Cß­îô?d©¢Ñ?ï¬þç7?_®¯'
àù?fpaË/?C˶ (Ø?~½Ð_^Z?[¡¸‹Eµ?ïå9#ÑÛ?_¾÷*Æ?<×ò²Éó'?-ò^'ë›%?g+Þ¤ ì?]½Ÿˆž%?ï"At8?5úXŽF?`Ob^/
q?qƒŸÊœ¯?ŠÛäƒ'`?ŒVéŽ§?…=Ë?z:ôßAÄÈ?b ¯Sef?dÁ'º¯þ?‡Ùnƒ±Éé?wL²'î
K?ï1ðhë©?yнñqõ?{gñ%‹?`ŒÅøQÈ?'è18N~}?v*=*TÕ¬AGN4FGL J0625.8-5441?ì¶8:ÈÀ9o¿aª?À:5C•%À<VH˜F@Úäå@o–@HÅl?¿o"͊aî?¶šÇ—æd?óƒ
€òç@	¡hðÚH?Ë&`¼Ù9ÿæk%^¿ê«ᚺ+¿ãu"Ód—¿ïþŒÍÙ<G¿ïô€d{AGNfsrq3FGL J0626.0-5436PMN J0625-5438?ïô¡íGŽ?N…SÑíœ?:ëFßn¬?3rTù©É?PS™Hîü?HR$!^Ö?ï̘ÏÅ$¸?{QyâE?Pô^Ø—7?d#¾§?Q~?uv€ƒÖ¶F?u3Á8?ï½-Hž»~?peFÚÈ¡?XëÍ¢ñkB?XMáµì#h?{.h=—h?m7R{D¾O?ïĵ¬t½—?XM 	[Ý?fYÇ+?J jnâÐ?r–üÄ~Ð?PÆY'0©?ïêØ1ôˆ—?`%"æcæ?N>'\Šiy?GžV8Q?[0[G8u«?Xª•˜j³ë?ïm){Eèå?8ÕÚH¨"?_$½Û2;?jK2æT°Î?h"¸[ݔ?0o`?mÅ?ï!'û"?}b!2R3?cU·‰p	?g
ÉO#?‡â.EÔÈ?z«~cRHÄ?ï[?xWÑ.¥"®?aV\?mæã#ÓP>?ˆ"÷s5ú?n_ c AGN4FGL J0626.4-4259?@1skÀ6qgÛ±lÀ:gØp¤®À<rZؓªl@ =é[;e?ùXñ°C?ÑIÓގì?ÊGçµ±RH@'í]f¤@-æ–Íar?èM!*È+¿ä'%ߍš¿áŠJ;tÈ¿Òu.`µ*¿Ü4%áæåR¿éäóiï‡ãAGNbll3FGL J0626.6-42592MASS J06263670-4258059?ïõ͟Z£»?J'ù`¥9µ?",Ñýà¬X?L)3'W?R&°FÅé?H/guÍS?ïãȏ®ç½?j¡Kƒ"í?8—Wbö´?EdÚÊsã+?i$Ú½¡?g>ùä'ÊY?ïl—0;d¹?‡£ŸòtS?^àÒT%?^uðÝ?×R,‹?†ÿþFz4e?ï¥'·Ûà?_›äþ?5?G]*mÅp?-a'ègtA?…Eèï!žQ?^î3BÛCs?ï팳¤?W_º*«Ë°?3	•=×+º?&ÊgW?`—@ÇC¢?UÕ{WœA'?ï¬õ^ê}?ƒ8Xc$ܾ?H
,\齌?W·I éK?ƒBÁZ‡Ç?ßlbª?îúç6|á?Ìn±x-o?iŸwúÄt?lWI»$w?o*7ꅣ?ø2Î}r?ï$âq§ì?z·Ց³ñ?RëJsd#?D^ߖÎm?šB¡
æ??zyKG}uAGN4FGL J0626.4-1712?춁	»ü¬À*FhEZ}À:¹%8ž¬ÿÀ</½ÿªo«@<ä1˜Ss@<à[?Â¥ýÖ.
¿¡K×ÄÍyñ?àwU6":@bÀõ(5©¿Â$ޜ-Ä¿æb­¿keT¿ê'v¹Ã?²Ò<ççÛ¿ç+Zâ#Ì
¿áã+~3ÆAGNbll2MASS J06262650-1710467?ï«`TdÂ^?{JÁÓø ?PŽp mõ"?D›¨™«jq?ƒÆcú?y»Cƒ|'ž?ï£Þ«éʬ?
Ÿªô˜•?Fª	"ï?M³ ¶›F?…´|"Ð?Œˆ¨jÔG?îê6itÒ?'1/#¹U'?kšx¹Æ$?d'oz¤?ŸEýjmiâ?˜ík5ª?ïAS²Y®ó?x>y4÷#?c%×`¾q?LÑ[³ï?•pÎ͗Í?w,Q̌DK?ï@yúÙÎ?ŽˆÛ¸?gÒ,ÚìÜ ?`Jà•€×?"ö{&Nä¹?ŒpåÔ_×?îÚRwØ9ú?®€m¿\¨?b'2ÞSÒ?ƒá×ncýU?¡.¯bP#¦?­þ­»&Á'?í¹}A@´s? ¶2ý9nd?yÙvO~?s¦×ð¨?°–~–Í3?Ÿ÷H'm§?í²êGÝ?–%Lî9<?'ˆ4è ,Ÿ?tÛ8"£ð?°H½a‰ƒ?•.É©ó'+AGN4FGL J0627.0-3529¿–ËÆts8À3ø2¹¯æÀ8êe˜ºÀ;ÚꃖøÕ@è7cnU?þM€†£Ð?¥I['Ý?'AÒiCæ?ìf¡t¯T@– 5T –¿¦áÃ\"31¿ßZžœ¿Ç¿à[Õì¿×Â"µí¿àŠEžoÂ0¿àæÂÂ1é1AGNrdg3FGL J0627.0-3529PKS 0625-35?ïÞz>N^?bn_©ê¼Ð?<§ÒVñ—?02Ë´¹q?nRе>,?`ø¯V×ÁŠ?ïàƟcU?r&jíp›?>ú¯ú6ׅ?KC/È?k]#y†C›?p´àƒ?ïl'`Gò?‰k:‰ßTs?oÕ¥ë4âx?z§  ~?±ëhüë?†m[ÛÅyw?ïV® Éú?p&—²yex?f×Âjª?F$¹NKk?'iÓžÿp?m-jƒ@æŸ?ï¬-Cô»B?x]	/2G?T‹ÚÔ"}?KÞÏÎi
8?'c3»u4Ö?uâ[µI¶?ï¦Vîú??ˆ¬¢F!³•?Q€X#†X¦?^ö'³Dâ?":95ÐwI?†ßá+ƒî?úŒ›?"FHŽº?tÔi´¯m?~~<üÌ£?˜ö"PÂUÊ?Œ¼âÈ,l)?î;—°¶A?†öU|÷1?wҁ©)Ü?`VXŒi?£2µÇX·?"ÇUæýª¯AGN4FGL J0628.6+6900?ÔK/.Òâw@75`A‰7LÀ:¶çºŽÜ§À<¯Tæb4@°´k½@j= ÿ:?ÀF¨0
_?¥0¼ê½µ?åAa)ÃÂ?üPåüéö¿Ç?›5ûåi¿ßN€2ÀG¿Ýߋ€Ò"w¿æîâ q¿àáÕ<ÝÖà¿å¢zH›zDAGNbcu3FGL J0630.3+6906GB6 J0629+6900?ï¿r·‹$¿?má'Žy?Uèµh. þ?E¯'9"?zÌvìÀ?kU9]èÀ(?ï†AîPÅ?…/oò:ÌX?gW"og¡7?j®™ØoŒ?ˆŠNvPVi?ӂ‡#?ï=‰æþI?…|Ù#Û?rÐû_!B¯?rf&ù\®r?"šêP>?'¥5‹ª|?ï6À>ìF?oMÜ5*C?~,[Œ€Ã?^	ĀLì?'£1Ü?kN®þÌtp?ïoˀ'­€?€%SŠåKr?k†òž}º?_Åß=Û?+cIëb?}cPïœ?¼U?VBp¬ª1?{:(=?€v2hàL²?¡ˆE<ØÊó?™$
]Û?î‰ù›âÊ?'Žax?}ìíŒ\…—?uU©GÎ?£°âµ')«?‡‡¾èÂþ?íÉDoE³?Šó¿Ët—ˆ?"?$:ïU"?{Ä$û¼?©Ì&ðÀÙ
?ˆ£½
Â8»AGN4FGL J0628.8-6250¿äfPxWCxÀ:vø½ì_9À9—Ú\ØHÀ<]õ£…«¦@Ûwy´!@ä̂úñ£?²ñLˆï¨D?¸¨xY­ñ?@GË $b¶@i}G(‰¿Ü¹­6/¿ã/¸ToÃÝ¿àÜßõÉp¿ãòžþˆ[¯¿â.•ßе¿ïÿîͨ"ßAGNbll3FGL J0629.0-6248PKS 0628-627?ïî"1(I©?Z¡¶Ù?1ЕÄÚ?'|"­¯Mä?^e˜a"tc?X™äC"/ô?ïÙøL‹E?qf§Éo	¢?AȎ#7ît?L>~:eîi?pÊÈÝ.
?nZU'¾A?ï´t¥³;?xè?%?_7âsy?pý‹T´°?}÷êäæ <?pˆ[è`â{?ïµÙñ‹&?\Aˆ+J@?_â•{ǵ'?<ocL[^Í?}˜™ÓÏ?Yp³- =?ï܅.˜?iIƒ$¿?DÌúŒ?ƒ²?8åêxtZ?nG"x©p8?g7â 'ö?ïŒL'˳?‹8ƒÕ6o?Tª£ì©˜?a"ëý[4?ŠWŠÀÎs?‰¡Ív"&«?Ÿ^]6?€~Ûq?h︴bÚØ?q)Ç=Y?‰!iñ±Ñ?|M"õH)?ï=K"°å?|à8Ž»>?tƒ­¦ñ5Ø?]9"\éD?"5£úiê?yn¹eºAAGN4FGL J0629.3-1959¿è "ôûÀ+U›=ÈKÀ8¦$'–GÖÀ;ŸñvÐ@ö@í®Š)@/L{ٕ2?¤þ€_G‰?²{婒‹@7b|×Â@¡ù5‹}!?îÿ5Ÿôým¿à;Ø»¿ã죗I]A¿âYÿ ^¯¹¿å•[|'˜Ë¿èK×nç>hAGNbll3FGL J0629.4-1959PKS 0627-199?ïðEÂyY*?Pâ«íÂXZ?!ß¾âÜЊ?ž£°¿Í?]8ƒÕæå?P}€‡yM?ïð(ö??j$Y.?&~	¦]?6öeåìµl?\ï©ïpÇY?i,ùu[ӏ?ï­Bõ·Ág?{dúÍ.{?ZÁ¼ø=CÐ?a]:N¯ê?WcÇ?y‡Cê/E'?ïê¥Ð´ç?Gšß†Q¿?+'¢Q?><ñâž?c©mb15?F«I6W×?ïßÓlôí?eŸŒÿ"?*Ьsàî¢?Ç\«ú6?nÖªg6a?eAprä»	?ïÑÄVÂÀ–?|˜–"{à?EÑn'[Jt?^˜Ò½Þ7¥?tc¦Û…ÿ?z
woӘˆ?ïƒÞ9Û?'°R"»rÔ?d®C½q?j^iò~äj?‰Üá	H<Õ?ƍÔM¤?ïÍgâì?fZY¨hð?@Ÿf>^?1xÒCk$?w]ܘ‡Y?ekõøevAGN4FGL J0629.6+2435?ïâŒxã…e@ë—¦zSÀ:w,50"À<6¯A@ ,IõÂdi?þ§,yێ1?ÆÎ'€L–‡?ÊÜ >ú;Æ@Ó#þâÊ@`KZS3¿ìõcߣi&?ïû0Ãj¦?°\ڗe¸¿Ü¨
»)Œ@¿å­Œ?¾ÜÊ¿åÁЄè1­AGNbcuGB6 J0629+2437?ï[ÔWŽ9ó?¢…õ)»¤×?Z±¨õ#M?P«¯Ù'|?'ä	û˜m?¢u°ªYÍ?í5ž¥û…P?¶ÐÇ"%à3?oCªêç%?{oÌûø‡±?µXíyЉ?µÑ*¶
Ý?îU»Oe²¦?"w¶¦âÛÂ?vlµGæl³?raíéy— ?§Ö´b_Ö?'It"d¾?èAŽ?{SÿZåf?c|pxÁè?c[Ñ!¡e?¡'bó´%?v'çowž}?Ë\?ž!6cp?s÷4¥/A:?jªŸ÷ن?¤©~•<?œFFPëV°?é"7‰Óm?ÅTkqèû'?£­4¶ú?Ž¥"~ƒH?ȔèÍçÝ}?ÄÕǽn`?ëÙþEZ?¦ºPÀ¯?‡û B Ô?~‹².˜ž?¾0©É›¯?¤××àÚ©b?í뢧X?"IÛB?-%4êXÔ?z^)2«²L?³-Y¡ÔH?'ôœØ9þ¯AGN4FGL J0630.2+3228?èTÊZÒc@$4D‡BÀ;Mä·¥[À<}Pǘ°@ ÿ€Êì?ÿ°g܈+³?ÏMyÛc='?¶"¾ì†?é\>ŸÍæ@Xg‰Q"¿âÄõ"+y?î°LÎå«Á?æÿN)X¾Þ¿èY¹Å¿à9™m$?—àèžË˜ÖAGNbcuNVSS J063010+322608?î†}þb?¦WÍLr¡?R¬Fñ´>]?JÉ­éº4-?§	uöV|ò?¦Pšn£?ìóÔ¨ZÉò?º2É+¶c?tcð p1?Š¼UŸ?·)^ð'¨?¸ägÐõ¶?îeÂ?˜ÿËÚÖÈ?tÔ`á2‡¬?p£K.õ?«…-'9œç?˜S¹ŽÍ$ñ?îà»oéX/?RWŽ¥ÖY?jIœF?`^oΤPG? R¤fÌô­?€MJCĝ£?íhܳÖ?±B(¶B÷À?cO2Nþ(?X‰‰ð7?¶Ê?Œ€?±74Û»
?é"$O·ñ?Çða2?€wMí["?Žîº†™Ï¯?Èèå‹?ÇHÆçÊBô?ë¦ RÛÅ
?©§ûo+?'R-}Ü6?xÞÄôI¿?ÀB]ÓDá?¨`c×?íLsE>oõ?œ¹.ÿ)½Õ?uUãÑg‹?qìÚöz(?´GšÎÙà?›¬ŠV'ÐAGN4FGL J0630.9-2406?ïS5b&‹À-ý˜ZÕ8¬À7Å™m#ðÀ;'>[…b@â³¹€iÈ?úw¥ôïp?›h´§ð}	?·³ìŸ@©"þ×áÔ@²¤­sì? Õú¿É¾¹ä'¼0¿Øtߚ¯Ä¿×{Ì¿‹Æ¿Û½ûx±Â…¿â™
'¡/AGNbll3FGL J0630.9-2406TXS 0628-240?ïó4ÓÏÓñ?P©Æºps?6†
9ÍÎ?7—¦?û?Sô՘å÷ç?J"Glûy?ï°Æ'ŸO;?ŒÑêg>ß?ZÕË!Ïz?p47¯Sž?€s¹Š­7?ˆË­·	¡?îk
  |•?¡Çú¸¿åä?Wå¦)ÎD?"a‹—?¥œ?¡#c!+‹?›ÊVŒý°?îÿþ_­?'(††íD'?x kÀ v­?a‡k킅œ?¬«ò¥Ža?5Âx˜¿•?ïíÜh˜'?\zKá+ß?9m"Œôõ?7@; Øª ?_–¬!'ú?Y'Þî¥j?ïD"zÈÚ?šBz@;n?s邑ʀ2?"ç(´"]­?'uÇÚ´?–mRëi­ß?îp¯rA?¢;åÌ\–W?‡à&îAÁµ?ñ5o U?¢ý~z?ž£ÔÇGEÈ?ìúÝèd>?¥â'"G.?"‰é ¶?t$]'Y}x?¼öëë\@.?¥"ôhúAGN4FGL J0631.1+2020¿ãäр26Ö@gŒSâÖÀ9kÛq«>À;—Ìe÷@@غÿñ@á">¿?Áݚzj)j?Êâë݉2™@'%ùŽÌ·@ð{Dü¿é7FBÐ_¿Íñ<†C&¿á§˜úà¿åàZéZ¢
¿çÀØ!ê‹z¿ïü-ãhÅAGNbcu3FGL J0631.2+2019TXS 0628+203?ïV….?ŽWÒ}O†Ý?cìÙHºe¸?W×u–[ÖÓ?›úÆâ‹?%j/º&?î á/
i?¥Ëék÷œp?[gò_‡ê»?içr¸Ý?¥­{Ú´?¤ÛHQÄ3?íl´6×?.RÖ?ˆ</)e€?úµ$¦ÞÀ?±—ÌzÚv5?šdafgâ?îÃÈãøÒ(?zˆae±Ü?nE£¥š"?L
mCn:ô?¡áífèoÕ?xÔׯÀ&À?íºƒà…øc?£¨ ·^ë7?vW†9kŒ»?n†@ès?°Æh—‰˜?£ *°÷á?세ª°0?¸'ñÂwË?qÓ«¯¾n?'«³'*U…?º½
w}:?¸½Má†Ù?ë:Œ4×"?©¢'Ûæ1?—iŽÌÒz8?Žîÿÿ3??À*"ô¶m1?§Fc̯Ñ?ì×õ4tü¬?•…x´Î|›?'.áû?I?g‰mÂEHU?¶ðpºƒ3?"gÙ»Å(ïAGN4FGL J0632.0-1032?î³ݦ0MÀ"ÞÁÁÖÐÀ9¢sۍZÀ;¶^	}@‹0k,ɸ@æ*C hÁ?¿Ø×á—?¼ô
ÔDe`?ú̺=~Ð?ùqï-Iå¿áí¾´Ü?¿áđ?h¿âJ/-êôÖ¿çaZž:Ø¿ì‰OŸz"¿ÚCTþßïiAGNbcuTXS 0629-105?á­*VÚq?ÄUËBoL?‰ÅóMõ7?{hñÀ~9?Û×{¹¬+?Ä9ô*E	?ål·R´z=?Æ2ªPÔ8? ûú–?Ÿ—='ª?Ó'Úæôt?Å1­?Fo"?ç¹í03hQ?®wöÓ"Õ­?¬ÒT0t>?š$Ô(i^?Éã¶="5,?©éCÓxêK?é7ç}R;6?F#øC"^?«o¯Ïá¶0?ŠYã#å?ÄDvšŒš?˜éï%óz?ÔíÈhl®ˆ?Á"ræù? oÚ#1ï?'k˜2
q?ä'$-Í?Á³âƒuôW?ÛlCiØû?Ëj)ê_.å?²rý¶j-ó?·-î7©Û?ßöý~V®I?ËáQŀ¹_?ã
©>…Õ?²/÷=´w‰?´z³^€'¶?¡¢.‹Ö"ç?ÔÕ7ÕYcI?°§WÒÒE?â'{3ýÞh?­|w8?»ÔnN3·	? 9¾ðj2?Ô»îwUn?ª¡ÕÉñMIXED4FGL J0633.4-2222?×OÂ]昮À+‰
Z[–)À:.MeÀ;ó£BÇ‰@Sϊí.@##—´½?ÁhÞ»·§?Ҋ¸?Ìô@"]Ä×5@f§€âéo¿åÛ1´­ò¿Ù§MKã-a¿æE'`À48¿êðÚ'ÿ"Š¿êŽ€á¼Èô¿ïÿ[ËñrAGNfsrqPMN J0633-2223?︧Tà
?u}wu:"G?ik žå?dMHý?vöîgø¼?oŸ¬Ì²ç?ïè$1½S?lRÛ/2?8é´3g^æ?DÌ3,^[¨?d¾˜¦tV?iò…µãYˆ?íˆIƒ½Ëc? Ë;÷(Ë8?™Q؈ï\­?'ó™«'^u?ªÒ{}óÍw?šÝäɯB?ﳘg"7v?`3yäÑ[?R=–gKÅÒ?8_FHð•?€Ò3S‹¥?]XDEÇbê?èó°"?ú)•ä?q©Ù6kl?hEÉ¡hØ?"Y0ó½Ò?}1 |-î;?ïªðä%¦O?‹LžYÀè?[~ãƒõ!è?s³¤RxÔ?Óê{?‡/ù'´•L?ìJSœf ?¨'KbBÚ	?£zÌ0çöÁ?—6"¥†?³ðAÌè¡?¢üî×ÓTë?ïoì´&?€v;dêÄ9?jÀ»Ñ9Ú?UÛýK­˜ù?˜Ú¾‡™û?~£­UK~‰AGN4FGL J0634.9-2335?ï݀çFÊÀ+ë[³"ý*À9ŸŸ¡—[À;öюÓlú@b
#Ôñ^@Ì{n5h?¹²áØçQ?´Eæêk?ø"Ñ ¤<@ö"‹ë[-?´ãAƒXµ¿çň4íH¿ç>—"ƒ¿çÖ!ªt³¿ïÿŝƒ‰¿Î‡¾ bAGNfsrq3FGL J0634.7-2334PMN J0634-2335?ïô5.`µ?S¬Zóé?:3Fzm9¤?6À"yq?QÑR~?Où´q¨Ë?ïÀ¸‹'?"rú=Ø?W'@§Œ?fÏÄq\*M?y¿iÿLwº?€Â0»+‰?ï¡îªm&t?{¯Ê÷uBþ?gŒ8nA¸B?p÷ƗöÏ?¡G9¯·?ujNd©XB?ïg{'Ϲ?lynù)n†?wÄÖÚOëÈ?Z¤¬Ô~+Þ?ŠWõÔ:ÑÎ?ewv¡J|¡?ïㄳÏQ?nÔõßñdØ?QvÓ­ÑÞÔ?Oçu'ü¹?c¿ã$f?kIB碻R?ïFµ¦-¯?™¿$
h'Ò?q3-\'N?ƒ:ð=(£7?'Ü'2_2F?"Š«RK'?ïMð7ØUä?ˆ—<!®?vkoUöq)?ywî	®à?§) Q3?"Ä(Ži¼?îUg]Ж?‹s¸}?'4¼û<"'?0SH	?¡0Yðÿ`?'SÚ8îM™AGN4FGL J0635.6-7518¿ëÅM†½ì,À;+Ë£!hÀ9"tnfæÀ<!™í|o½@ûPO£¬B@…×ÙôÓ?§zGÞÁp?ïé:g}?Ýò@úœñ@kº%€B0¿Ýﯛ
·ú¿ä†l@E‡¿égÿBÀÅ¿é»Âîýy=¿è;å¿ê¿á["{L§xAGNfsrq3FGL J0635.7-7517PKS 0637-75?ïüe|d27?1õ~¢­P?Ð?{: ?^eËR©Ü?8 Ú{?0''ß֝˜?ïì©{äÒÓ?{B'ŒYæ‹?#Ì¿¦¶ÀA?4⚖Á~Ó?b¸4"À?zú­`˜í‡?‡S@?~+¡Ë#Œ?[€;;½?a9"¥>?…,J‹¿f]?{áèB<?ïþŒÌÆ[ˆ?<¼œ>öó´UZŠ÷>äˆ`|´?$T¾‹až@?òޘ€Iª?ï÷Øñ•¦g?FˆJ]lW¢?î`ô ¸?r°¢·n‹?LþwwpÁL?Dôô±×ñï?ïΫälH?ƒ'="¹´?9_NÕ¼ñ{?M838R?wÔuØ0?ƒ5`'_'?ï.ÅXlÜ*?Œø ²Î?i‹6—#B.?n7䶌
Q?–õî"?Ây?Šç79Û¡"?ïûÖ÷.[n?4NÙ²Ys*?:Y«ïô?	b
¬Ç×ë?<yÁºÓ¦Ø?2°æŸ3ÒAGN4FGL J0636.5+7138?Çó`ר•W@8~´Øº@ÙÀ::ªù›À<[@ےbn@Eˆy`¿@¨[ü€¿?¹há?öe"?´Õ³{B¤?÷1^µ—ý@àl
ë?ïë!äVV¿ç5A•Ì…¿æwô˜Ã°Ä¿æ.ÕÀç;c¿èï9©nù³¿ï߄¬°AGNbcu2FGL J0633.8+7132GB6 J0636+7138?ïó
*?2Š?Fаü°#Š?8µ…¿Z¾?)ºxF/%?S¾JøOž*?Cʃƽš?ï鏑5¥‡?g`÷¸p
à?8͜Ðx_?FU\o[Û?cV»<ÈX'?cˆU(m]Ú?ï¹¢úò$?h1¨‹{Q?Yw%Ôb‡?D!ËÀ?|éR9ÕO?f6ɶYþ*?ïóTå¤Mì?9¶n]%àÅ?7ãMµ®Ÿ`?¶õ›v¤¢?S]a'âÅü?7qþ{ï°??ïç³i4³!?Wx64ÞÖ?Gè5}Ò?9—vO;7¹?bR¶f?T޺흙?ï²÷™T$o?'¾[Tž?Lê,‹¶Þ?Zý¹'^"?svöP±£?€Uiú©®¬?ds5ñ?y†€©ü2?i×@+Þ¼ú?iW-´Ô=›?‰ZVÎóâs?u_Læhw?ï×{¶üù2?]xû€yx?S&abÎ[?>nq`,:?nõ\ç\?Z"Ašš´AGN4FGL J0637.4-3537?èámz½	À2	t²GÀ:ž—•}À<xŠ]¼t@tècV;¡@
Ù©T"?ÆÀéª(2#?ÃuG?Y²#?øB*aÓY¯@2Ot\sH?ïÿôÂ_5›¿Û‹4œ>ån¿ß<߆d¿ç&zü	¿ßԜåS\¿ïÿŽ‹HÿAGNbcuWISE J063746.40-353648.3?ïtÈá}?''49%
0?U"ãŠø?Nè…ô?Œð˜ŠÏ?Pé¾~b'?ßÞ´?_þâ)a?a·'Ϊ9?deŸ$ÛÈ?ƒ©ÝÂ?{Ïû"œa?î•KPWӞ?˜
´áƒ?vÙ'Ýaü?y]×ßÂù/?£Ð&lLß?—T'VîÊ?îß¡
¸Q?tTq•S}?}ÌjlÁ?]"Él`
?œ¬fÉåF(?roshH?îÞkcXój?"		Tl²¿?pͼ×!g–?f£ÇžêÖ?Ÿÿ$VÚ(ì?'ÄÝñáyð?îå :È}Þ?›2ʪ&?y›þñ[¦0?"YéA¢?œäøëù2½?—ªì
•ûæ?í¿àj/ëø?òÎ¸K?'¼·û2Q"?k×ð9‰õ?¯RËZÛ
š?œËúfy`Þ?ízsŸV?=9mö,á?Ç™º¯Fˆ?vÛËìrǂ?³rIsÿe­?‹ý=äÚ8/AGN4FGL J0638.2+6020¿Ûl›ÍYQ@5Æ՝Uæ¼À:Þ%‰ýDdÀ<'û_‡O@&cõÑb@ÿJ˜ª†Q?Ê"кm#Å?Íf¬¸ZO@ŒþùoÃ@hgÝ	¿ìÿº_⾧?ïû';&F¼¿å½xÁ‡Ê9¿æü»bJš¿ïöÃÁ5iï?Ä1ˆ8HEêAGNbcuGB6 J0638+6016?ïYcûkàh?<ÇþÔ(?w?ðàB??sûßbeJ¿?Ž·þlT?ˆÅëi[?ïJ"~]È?'wKè–ï?~zB"ë|Ý?ƒ÷
B¹
?Ž!¿8&Çq?ƒSÅC¨`±?î±`4É
?'NXÅÂV!?€Æ>q"?{vWãÕF«?Ÿðó
à?ŽË¿re?ïM÷H[?u=lY[ò2?Í®ö­XÚ?l,Rêø¾?^Ó"ôf?l€ÎûZé­?îF·	Ÿ™–?¡öSçA­?0
i!Â?†»m(øG?¤HŒ…'?ŸNõ…?2?íҐðõîQ?­­ÅÈ"í?—æR@$ï? Òe
ÿ…?§L}ÅÉ:?¢ÉòÐ_?í|Œ½D?»ÁF7Æ?"¸îV[í—?ŒYˆ¡=–¨?­Ù°²ð?—$ŠÜŽø?íBœQ|@æ?"·찞Â?¤¿è¦ô¼?ŒÒKélӃ?§RÖ%`ï?Š(4•éAGN4FGL J0638.6+7320¿ïûÍÈs@9ºùe²À:ó˜éprÀ<Mš#×v@!T‡ÁªÛ@-»Å=ŒS?¹¶2‡?xmّ2ö?»£Õݗ E@•§ˆo¥ª¿ã€¹ÎÃG¿ç¡L'HD¿ë¾Àdß}©¿é£"î^íÌ¿î6±•+v¿ï«WÂ3Á£AGNfsrq3FGL J0638.6+7324S5 0633+73?ïãyÚaŠß?{e¶PÔÕ?MÐö@ñd?[º;¿ºÃ?eè(&ž}?u']	ô?ïߺîí‰?t?Dþ%¤?B•†—.¨?RnÏ@â8?k œ«Å?q•TÈ|®™?îâçßUn$?˜+ëºO|?a¥x¶§FØ?lÃp^‹j? ·*~LÄÑ?—º?_¼?ïð³»ü€?@Vòº"Ê?F
–ž}˜¿?/ØëÀÕ?S'½3}?8ÀñßÅ9¾?ïØ]Ä×5?yC´¦‹}¡?YcZOƒ€?\q´Ž—§?jðµ=›¸I?t#ŸÃeÙ?ï—æ(h~ï?"²726Ø?X»ÀÉ%þ¸?oã†r‡F?†îýÜá®5?'úí7¦é?îwS•ö™?£.ä*G¸b?h‰â-hº?q L@íPf?­ì¥SbÞ?£œ)Z±?ïËßBÊL?fΨ'm?ešsHøók?W?¡Eyÿ?n†yŠ:@?_4uˆ,[ÁAGN4FGL J0638.7+2753¿Ú%§TYc@##_€™À;K§*{ԍÀ<œLŠN@!Y¹óA‰?ûø=^/`@?Ñ&ö¶|?–;֚ÖÛ?õ~…&E'?ôkڔ5¬Š¿ïÿï¤h)µ?è%¿âÙ~Œ?ï÷€Õ}uw¿åR÷Ù.Û¿ã×ýsº?Ë‹i*;AGNbcuRX J0638.6+2751?îi˙¾?±°)µá?Tˆ)lþa?P~ÜšrÏ?­øÙÀݪ?±ùÔº#t?çܨƒñ?ŒÖ`8=Î?"]+PÒ?¢YM?hW?βZÓ½?Ĉ›²o?í&b"uK?Ÿ©vXa?~VPd'Ô?}J™ŽØ?´ç†× ?ž#`_ï²^?ë¤\^¿m?þ´~áØ.?Çö;j–?…†míÄ>3?¾­¿Ák'?›\5M#P:?ì{ÕHà¥?´bx'ó>$?e"§žaÎÖ?aJä~Ð?»x@ƒ}Îb?´IÌvØÓ?áih^†Y?ÏËL2ø?e­ÿŽ2a?¥'ý…qp?ÛVÓä÷™ˆ?ÎCAÄל?ê`rŒö"<?¥p 3Þ,?ˆÔßY±?'VQÞHè?Äðç֊Þ?¤¨¦¸S?ç'›XE?²_R‡Š™?"èÊjƒÔ?"q}Ôh¸Ö?б$"§¨Y?±§Bé»nKAGN4FGL J0638.7+5658?½Êž@4ÓDZ¢äÀ;
X;*xzÀ<›b§K3@¡)œ±|@¿¤Ùš;?ΐ¸‰ôµõ?ӜqeHO@‹"˜€"æ@¬@?¶#h?ïî¤!²Ø¿æUïÝëÙ¿é(ÒxÞ¿äœ¦°)¿ïþ–¾ßú¿ìÝE ž³AGNbcu3FGL J0638.4+5704GB6 J0638+5701?ïÄz<ÿ\9?r…8	Îk?j«þxÑÚ÷?dÈh›J?plâY6Š#?d¦:þ÷(?ïJ©×XP?'™	
á8@?|îŠ;HO?'¢w‹K>?ŽÞ‡ÛGå?‡Ã'vî?ïcAën?	ÜÆÁ¥9?ybÀ£áT?vhý½Ë?—[ª…Dæ?‹¤©"¤Âa?ïAÌˆ¦¥?mX{ؽÆ?ƒÇ©ø?^Ê*³ÃH?‹Ô|Óìúà?f8ÒÈz×?Z‰í?€yb¾ý[?ziTDŸ?r˒Ù?€_3LI¸è?uc8|zÒ?îªãäº?§Ÿ'/†¹?'ûyªÞ1ñ?—Nw€kÕy?¥g"ö²ÿe?Ÿó	m)2°?î¡ÈÅ+BÏ?—‹†+^Æ?•³Kíwf?|k뵃?¡ð½At)?•u.ILKÉ?í•üš3·?Œ¸YÄ[?žG:½pWd?s³à#?§ŠÂÔ4üà?‡låÜhKCAGN4FGL J0639.6+3503¿ä^à[R"«@)í¢Pø@À:Yã|;ºÁÀ<(ѧýàk@2Pó€Ý@9{ßto>?¿0öíݓ™¿ª¢ÒÛãÐ?ëu'Ìö¾@\T‹GœL¿á˜
þEjÿå¹ÝaD"ƒ¿ì/s‹¿ÓÄ{ÚìË¿ìÈ÷?½X¿Ä	´Ÿ.ƒ÷AGNbcuB2 0635+35?ï:ao~	"?¹eMU¬?"üÌÏ*?¬¤6ïL»?Œj×XNÈ%?«&x˜JÃ?áC?–F´ÊkU?`Eò©ÞfÏ?rþߟ²jO?‡
ùµM?"§ºˆkb¾?Úl·R?"ãøµ‰?"¾™û‹ž|?†ß"µ
6°?¡5KÙu¼@?çóV¿Îc?ï´T6tA'?c.‹°¯)3?^Ž—Ééû'?G=rMÕ?~2>Ò´Ôo?`£fç]¤M?îè¤9ŽI¸?§ãö. øê?'ºø.½g0?¡-ð£øŠn?0€–â[à?'ãHTѕ>?îÌrvŒq?¦üvìBc?|¡
'%o7?–ü–±:?ŸV/	ùk ?¡šH:2T1?ìô_ÒÝ?¢^9æ?"jié%>?
›Cô¾²?³Bg,Úµ‹?ž×˸¸‰B?îÿcDóÏñ?‡«8†û¿?"¡w$u?sm_ˆ2Š]?˜NòwtÈ?""<†Ž½AGN4FGL J0640.0-1253¿ï•À›ˆ~ŒÀ ¤€¥¬ÍSÀ9é/bÄwÀ;õ­§m—³@""†ÖHv'?ùÜسŠÜg?»~b MÓ?¢6,"9Ø`?åÛb'Ő?ù×E÷†	¿éx¶Ë¿åªy»­Á¿àY!95«³¿Î¹©™ìУ¿ØÃd£î‡2¿¶@¼ž+y«AGNbll3FGL J0640.0-1252TXS 0637-128?ç^õÜC@?Á®}ºüý?lŸãg)?`ÂD—±?Ñ
»ãÎú'?ÁŸ¶Ìc?æ ^DâeÄ?Ã8ؗ8ôÇ?x%Ùd}¤?{´•NSp¦?Ò^¬rF¢?ÃtÀžw?ë{*›è†ð?§1²døš^?€E]Áu?zNZÄXG\?Á8©²?¦ÿãrÓ¢?èD&×@]?§ZÆà<?Š¬j–¡Ã?s¯P'?ÍD›¬T˜o?§<páx?âN©®/'?ÄÜÏïl	?{"ﱏÂÉ?iø´ºbä?Úö äã*C?ÄʚQ"6?Û©Tù'¹½?ÍVS–!Œd?@®ïϪ?Œ™ol
^&?áæRÇo#?ÍFFÖ~&w?çóŽ¤ëT?±ÍçÉMGy?ŠrMë¿Wù?ŠJic?цs!4Ù?±wÆÝ:?ßX‰Â?´·:ۜi?›ö"æw$?á™$¹#Ì?ß-?å_ì?µ†Ò'Ž±MIXED4FGL J0640.8+2432?ÒՉ±'f@!~O3Cú+À; C÷¦•+À<r2ËŸ@!^Î¥?=?÷"]wª[‰?πl÷м?ׇS±Wü@@ÅEÅ@Ìÿ¹^0¿ïþ›A9†?ïÿöµš?d-o¶•h?ȯD;CM¿Ü\O™-
¿í1}‡ AGNbcuRGB J0640+245B?ï.Áx©?"é›Ðۙ&?\Jò÷i½Ž?RܱâéX?˜c/þŠ?"Q'L͘b?íi1Å{?½'75Òö?cIWí¾¾#?sv
 —Á?´'–Ñs?½	n[Ûр?íA,=Æ?ŸÇ¿H(°?3ʨr^ô?)h6Ó¯?±é«k›\ý?›XþÒ—?îÒìS¥Äu?"W£7…Y?hõF$½Ï?S‡`+ª?¡Aæd¯tP?ƒ|ß.c<©?î&¬Ä«?¥^«a€?k…8°i?hB"®Sі?­eD‡¬LÉ?¤ÑAÂ\ú?ê@DW-B?ÇNP3›?~gì&Ís?"¸joS'±?ƯBš¦¬?ƛ"?'?ëP£uÝÊ?§|ј?'+ק˜š?,<ÉßÝv?À—÷D¼êÏ?¥ßýæ?íRJÃä
?œüwó:ö?yuËÔ]?p¨pߊ˜?³ÖS:¥óc?œ vYWò÷AGN4FGL J0641.7-0320?Ø?nù:œ'À
oZÎÀ8mô¡',•À;%ºÜ	€²@Îü<Ñí@nòÇ2Y?°—Uq¡'ò?Åß_vˆš@L{‰
Z\@ƒs¢¹ÿ¿ÑyÁ¢w8Ç¿ä,0àrœ¿çG–,&Ïx¿ëymª'†¿ïy?n)ÿ¿ïû!sîfAGNFSRQ3FGL J0641.8-0319PMN J0641-0320?ï¤nOF—È?€t_îë<?t:·L›?ob®&•ªE?yŽÏ‡+sÇ?tñ'ëTÇ?;zæŒ?¨0€9Ab?PcxB'k¶?b]±›.t?¤`ð‡q`Ü?§Ô)ºü<?îF#*Á?žNÃ'Iªu?–"AÕ|8?"Ê×0T¼? •\‰rùÕ?–Ø΍ ?ï wÅł½?iBÚê ?YÒÀùý?B40ýi*€?"Â
òc'?f©0h8/À?ïRD‹8$?‰/sW‡ó¡?y©Ž¯‡Îà?q$öŒÀ>ˆ?Žš<'‡?"}`õ—?ìI:¾dK¦?¾ðQÕ=gG?e'úÂÙ?&³"µ¸Ã?½	™œHËv?¾—Á¹YŽ£?í¡	o.P?£#M«?Ÿ¤½‹§˜ª?˜»Œíë~´?¦À¤5¬?špjÝ]´?ïu––@/?""Þæøš?rS"øÿÜ?agìj¥Nÿ?šÏ¸JÅÝ+?'á¥pÃ.ºAGN4FGL J0643.2-5356?ê-ñðÀ6É/Ÿ¾wÀ:m÷hÉ™À<qދ;2@ÊkÃr†@"NÿA"?½>™~ýÈ)?'I©¹™¶—?ÓÿZS2¬û@\r˜£ÐT¿ã[m¯0Ô¿ãr2aüõ4¿ã£ð4°áµ¿äžh5s¿ë#î¼á>¿ïÿ÷1$e:AGNbcu3FGL J0643.4-5358PMN J0643-5358?ïôP*ԃ¿?M7% ?9©ª"eµ?1–'>7ƒ?Põ?tÄ~ô?FÐ拙1?ïì<
ø;;?eÉçÆ-º?)Ó8…îÙ?8Ûºº°äú?b2Dɧ4'?cÝçCGÓ?ï·|ª—æ?rç\{o!Í?[ӄ'ùG"?e=œEØë¬?}}`""£
?mY©Ê€J ?ïðw˜¬£{?>×݃Ü.(?1¾(ùÐ\Ž?©+"$?Z¡D–,†­?=+*±§Z¿?ïÞcÚè:ß?ƒYy˜C?‡?SÕƒÎÓû?aE‹tBÀ?g±—Ô}ß??~©¬Ù©?ïÇY´ý"?€ÔyäEl?9ҙ»g2?På
´ì)ã?zÛ©xýŸU?ø憉Rï?ï…Ë	dhñ?}jh-P–?c%*$G?hänýØ>5?‰Ãó/C+Ò?ypÿópõ"?ïØ=ëëB{?[Y8Ä*[…?H¾³àéÏ?5\õ"˜?pàr3Š¯9?YbVHÙAGN4FGL J0643.3+0857¿ï•y~ª@Jf:Ç|+À8Eöx—ÁRÀ;w…@˜Cz~ l@ê#ÚЛŽ?ªeŒÄ'?Æ¡°êC*L@g:6\³_@žS;¿Õd¾{PX]¿à¤¥0¦ù¿çPáïɧ¿èó­aL¡¿ëlb©Ã]¿ïÿ†}³	,AGNfsrq3FGL J0643.2+0859PMN J0643+0857?îöï=:2?¢ÿ¥Ùl8%?ŽÈó6^"ò?ˆÙþsò?'½ž½??¡2öå^›?îпÑoQz?¦çu'ôÖù?a0Xû«DÚ?r8ÔNÍ ¹?¡àýWu?¦œ¬W?í
8¤Gƒ³?¨-˜—º?¥V%aʆˆ? w?y(2?ªP\Pó>?Ÿ»à9'Ó?îí÷Ž,?€´Ì$?p<+´ù™L?XKƒ<Ì>?žOö:îä0?~é"?íÜìÞÖi?¥‰ÊI³Ôä? ÀÚOg't?žZS/=_?¡pWÏqü?˜f®R?ír:b°?»"
Å?j?q—¡ÅS°þ?€¸?Ö;Ò?¶ô@k©?»$——"dY?ëÐ/TMM?©Ï3Ys¹¶?°»õ)Cb"?¢èÒ$Æ ?°Â6X&"?¡¢Ž]@ñä?ìÓºw4À?døÖ£Û?‹¨Ô?ÊÕ®?x<¨V
¼K?µò?¦ÍI?›–»øüñýAGN4FGL J0644.4-6712?Þê'	°À9‡ºùe²À8½CwN7À;̾&@Ü@œrêƒA@K²™ß:?¥ìAº¾
?¶ïôAðe@ì-BXj$@¾&-f?¥?Ù:!¹ä¿Ûn¤éb/¿âV<»È¿á½4ßݵ¿æTd ;ë¿í»Šàn?NAGNfsrq3FGL J0644.3-6713PKS 0644-671?ïÅ·nõ4?¥bàÝÁ`?Yº
	'¡Å?†Îƒè»A?w!ɐ™¡?Ÿ1SC­?ïí/YùŠ_?cÑ˸kw?-gd]Ý?AÌ!³"?`ú4ê"À?aÐmSà
Ý?ï¨êÚÔÍL?›íRºñ?gIE s‹?tæú…0C?åïÈÏ6?}ýö'ÊsÓ?ïû'5‹
v?'Æ3'Ò…N?ÞüOTw>ójÏ×3&?@¹9¿e?&¥hOÑ?ï'èmšÀ¿?¤5Ñç÷r(?_Ž›‡…ö?t^ªz=ç?‡T"‡×_?¡Õú ¥"?ïÒUÛ²Ku?|ÅÍÚ?G/º¬g?jƒ›³«ºÃ?sïˈ?vk›^̅?ïzŠ´	É?Œ\â¼Ê·y?q ¿`ÔV?|/f"›m?ˆÌó@Ýsl?†W%«¶&Ã?ïödnÆ?Cð$c¯n?M°Ç o?^¯7!mð?Ršh'œÿ?C5u*'AGN4FGL J0644.6+6039¿à \›%N³@6ÔÇm{À:_þKÊÙ®À<'©1½n@'²'
@a× åÂ?»c òÏý?–ÇùB:{ì?à<í'hr°@Z]ÿ—¸?ïøC""~¿êxdàTi¿áZÕ¤ãc¿×ðŒma,¿àШ# 9¿ãzˆ\ZsêAGNbll3FGL J0644.6+6035NVSS J064435+603849?ïô<Ä<ÁŽ?E¸$¢Ö?4%BM/a?$—Uî[TE?R}'ö×?Bý:5óÕ²?ïân,-…t?q§K0&·?;oDÀ²íš?Ec«O'Å>?j#ë|OB?oÉóÇjË?ï§Ô>ž:?yá0¤ëÛ?SOGPú?Uäù'jpk?ƒ¨–ü-?yC¶!à['?ïÙ¤‹²s?QcàÐfì'?GU,k"?%­_ó>į?p'SF03?PºÂ'?ïêQ¿²ªY?VÖ°ÉÇ?Aè΋YL?4ÜÐn'h?a4hða®?T›å^°?ï¨p1ÉÚ2?"kê‹Ûà ?LÞSxÅî?^O'äG«?"a¦
õ?''^ÀîZÜ?ïN«·ShÞ?‰œ¼oϟ$?\šï´Ë$´?aŸÒoÛN€?"`Ú~ ?ˆªÍœÌ(?'Ÿñ¼?oÌZN鑻?aaiQž?HY_b¦P?‰Æ…ôº•?n62(yAGN4FGL J0644.6-2853?î«£K7û‰À,&o"5ÒJÀ:Í»DLÊÀ<iŽ2]J^@ Ó ñ§£?ùdM‡rO©?ʈBZ¨m?ҁþÝÁ×@	bçcQ0@
hs[í¿ïÿ› 'V‡?ïó¯ûî|?ÀEýz¿ŽÌ¿Û'@5пÏ	IÕ·4¿æ²d ï&AGNbcu3FGL J0644.6-2853NVSS J064443-285116?ïŒE$rH?"¬ÁG;0‹?`:áï??SÉkÕ['?ˆè
Tƒ8O?"pøóâ?カç?ƒ"€Ë#ú»?SHý+°¤?Xƒðü‰(_?|¡å[¤—€?z"aô:?î¨!͍ń?"Žg¢«¯ÿ?ƒ§<Iþ?ý?ƒ;Ûq'·? "¸lÌ?'¹âæk?î@ÏàAb?ƒ¦_ÓÐ?v>õþ±5Á?^?ë<ÎaR?©+#:ìP?'}>?îÿÍŽqP?–¥ÿ@'ö?t1S"C£?jcC~qˆ?šÿñŽäd?"®üfÊ?ï
ºÜ=?žt)o%'?tWÄ¿…ð?;†p+"?—HW}W~?–E&sÞÔI?íR‰°Ô…?¡ÊåˆXÊ4?'CsI:]?=~"¶1'?°Þ†à¦ÀÁ?òÿm?ì"éòLŽ#?Lî[‹?hהYœ?q£—ð²:;?¼»¬uá¥ï?œ‹ÓMén£AGN4FGL J0646.7-3913¿í›_Ç»ÀáÀ1›ÜY1Ê}À:JiýʛšÀ<HÄdH~õ@–ìËÅ»¶@wdã¯ga?Ä:DŸlAr?¯'ªa4oÁ?ãzksù@	‹–ßU§¿â§´«å¿ç¼¯ŒwG¿ìc1" Õ¿è«k…L¿ïþrÎ\¿é¡–R½<6AGNfsrq3FGL J0645.9-3914PKS 0644-390?ï÷7å}%?|ñ'T]?EqIX+ºå?zíŽÿXÛy?<Û­x¹'?VT&!l¬:?ïØsæp{­?váÜv|÷?G9ŒªrN?TÕ^òÎÆü?pÞÛI¿ ?sӞS	ã¿?ïkÅb+×?‹ö>y'†?qS­yFN?|>U,*¡?ŒdÐí¡aB?†"€uÉ??ïÜG«)'Û?Q'^\5ÆÅ?Q¹7üì?8'fÉk?jï÷ö!	?L*88?ïô-ºVN?u5Æm-œ?>µBZ²?Bx{Ê T?OîvUO¥%?uõ':?ïzj2‰ü)?˜wJEWÎ?iQé±{äÛ?u·w[\?‹ù§þv?•‰1¡Ë‡Ì?ïÜ&˶?'ž_'g?yHï1w"?ÝB(P+?–:ò8Nøw?ŒÜҘ,¡?ï•òZx~?tOðs Î?ln	ì:—Ö?^x>vy;?ƒgçºT|?oÍÿˆ$AGN4FGL J0647.0-5138¿îi¸qåºHÀ5—Ø'sâPÀ;•YÀ<¥øZQ
@!CŽqwÛ?ú7ZYè©¢?ÏÌt7_gÅ?Âm9©Äßî?óTsۍ@­Ô€Jh.¿çX-ˆÏFû?ï‰ü¾, ¿åþ‹#¼H?Ò$Œý)¿ä6Ÿ™Û¿ÐÛPž(­AGNbcu3FGL J0647.0-51341ES 0646-515?ïòAZµ¥‹?I!Ĩ±?&Ë\N?îLк?X£è ½x:?Gt^~wZ?ïçòãÚ'?jÐIy[º?0>7®¶?='n?fÝ%B®H!?gÑ®e.,?€]³?z6Z%?R¬^Çþ]F?;çˆm(n?‰ÿ3Ív?yïKÉÍT	?李S̜?fˆëè?R*=ÏòÆ?=v× Ýv?ƒÒcH|?dôÞç¿û?ïåHNx^?\…+Ûs?7ˆ}Ðô;Ï?+σ¥l}?gÆ¡Î*°?Zµû¬¢£?קּθU?†	F4H°>?J¼s*
?[¢°Q?'òK;±"µ?"PPx´ë?ï;ÊĽg]?…g²˜t?XŸåqŠ
?LCüÒAÚ¥?–ü©
/@Ñ?…ZuO4?ï%Hd{]L?'ó
«?d^k6*©?[5­ÅKRR?˜Ë&¦i ?€¶[Ì¥y¾AGN4FGL J0647.7-4418¿æ^
uÀ33sâOëÑÀ:Ãf½ÌÀ<"ERðgÝ@Òÿ+ní@='¯š?È\S}€‰R?ËW\È­ÙB@·kÜÇì"@äNs«s?äšF½©™A¿ÜùÀGƒL¿ä¢­>'¿×˜Wš¿ëé¡éÛÑ¿ïÿý{ÁA~AGNbcu3FGL J0647.1-4415SUMSS J064744-441946?ï:›-ù?ƒú}>*Y?{=š:äb'?jJ*÷÷‡.?'ðf†2?›Pˆ@œK?ïnÌ¥›Â?†YMÍ^R?r9ÜH)ŠI?s­ŽÒO?‹[Þ¡V>‹?€ûf]ð?îüuŸ?æ	4?'q·a-|ó?'¥dš0²Ã?—8ppÅ[?‡>éBûÝn?î6ŒÏ0Õ5?}*$`Å?¸6µÇî?j"/¡Î‡e?¤©.ÿE:µ?x›j‰s¢2?îV©Ñ0oñ?™	ÃUÞ6Š?iÎĬi?m¹8¿½Ü?£P{ۊÙ?"›˜G@"³?îa©®?£ÜáxóŠ:?‡!æ›FÄ?Î@óú2?¤‹É[Úð? ¦æ³M«Í?î"XÊÇd?˜—ª2sL?Ž.&ü:šþ?‡B>¹°,±?¦N铟2?"Ò°=T\>?ëiß A²?•VBÈJ³¸?¢àljªÄ?ˆŠÀ]´®?»@Ÿ9cy?'‰ÃbÀ¿xAGN4FGL J0647.7-6058?èvÇ¢kzLÀ7ï´_½ŒÀ9ÆöÞN«À<R«ÿÍ«@ g-Å`@Wç^j?³(¤9Ù?¥ÐKÉt?ñà^åh¥@ו9?Â(mÀοæ8éU™¿ænÖâÐDQ¿ãIŠ"-Qr¿í7!ŸŒø¡¿ÑH¹­5WÑAGNbll3FGL J0647.6-6058PMN J0647-6058?ïíwB½Ðí?€Æ ¤ÿíû?3¶á‰o?#}·í+—?`ü*Ø ¶?€ÁYîˆ/K?ïìyZ+g?fR:YNB?1EЭ]Q—?B½¦Ÿ'9ç?a]ì	>?cD)Špç^?ïÇcël—?hs2N>ƒ?Y}'u¸'Ë?c»6ÁïäS?uîÓw÷¤?^Y‰+]áè?ïô'ït?6ø.©ã?4ŽrîÀ?ϲ¦V3?Q¸¡EWF'?2óvc'	?ï忧AÅ??kEÁyIž?BešÖí?2êtC:2?e¦òòû?jÐ,TJ{?ïɞó(^Ì?}Ö¦W|š"?@±YëɘÉ?RBnYÜ•?y[H?|U486•M?ïŸtëp§?yT³DhJN?]÷l
"ÄT?WunCåêù?"d}EÈ?w r<¸?ïànöéç÷?V›=³<Ìp?OMdC—Ì?=ÇcÔéÊó?g­µÍ…C?R•4†Ï¥`AGN4FGL J0647.8+4527?ã8ôœä@¡@2_–لÀ9ÏÒ␃pÀ<žßS¸@"mðÉVK@/»õäô?»ïj0 [Ö?º®?-÷?øäӛ'@¿ü¯¾¿W…ï(þb,¿åýÞó?þ¿ë4úqK¿éªBÿY¿áÑCõ"Vl¿ïÿçáüúAGNbcuB3 0644+454?ï¸Ù ù<ö?u-#ö¾‡?n€Ì­á?eê±'ˆ*?tRÉmdÄ?nÐA—Á$'?ï0䟄ó£?¡
¥4Knæ?€`%â?ŽôâúègS?'Ù»ø³c?"¾©LGˆ?íý"Ùýs?›ñ-éÃÆ?˜I&…<ú¹?""}"'ƒ?¤҃?'ù>K¾e?ï`•ìæÉ?x^×;é£?‡xwí<þ?n*¡ºµ~?w­‹"òf?m­d‹rŸè?ï[£qV%ô??4loõ?ˆka31í?Š!Œ1¼?€ø¸?Ls-?|ß0LJ	g?턾ÄT
ø?³Ì°:V?Ï_'£?ªUBÈ>­?¨Ìd1­Í?¤±Îr(n?ìU¯ñ"?¥x!Qq?©s¾õmÝ?Ÿi3œ•?²ssp3E‡?ššªô\t$?í83{閘?˜¦£*WŒ?¤}U‰ú^?'¾™æíö˜?§ÿ¼éHç!?Œ=í1­]WAGN4FGL J0648.0-3045¿Éˆ¶Ä[À,M‰ÎJ{NÀ9^íÌ ÕÀ;öJ…_Oò@/"⥧@tÁrüw?ªc;
Ȭ?À¢½¯£q@lN¡MÃ@.y¥ˆe??Û¡Ñ@ÏÓè¿àXR§lÀó¿èl3/u¿ç2,ئã¿çØì`¿ïÿî' ÇAGNfsrq3FGL J0648.1-3045PKS 0646-306?ïîñ*á;U?S—‹µõם?Ad,	ÌgY?9ÌÍLŒ¬'?Yk"U9{Í?OÉ÷L0nµ?ïïQ,K0?h:hÛÝs%?/D§€ê??*ÞC´õ¤?]u—'v;?fvÉ̙v‹?ï¨ê«Qt?u8é25•º?bŠwëYŒÝ?f¯knŠ6?Y'j#s›?qr[Ÿ0…?ïö2;¼n±?4G6uƆî?,‹«
Ö°?´‹°Œ	?P
R#?1Š¿­cA?ïÙÕUKOÎ?k\}ÚûQƒ?Mgº:"ÖD?H¢ÖTçþ?nм<OS?hE¬òח?ïÐIîØݟ?$‰Zì?KyH?5‡?mäcTS¸?tkß}¥±y?|"¥¶!S|?ï[4ۘ±V?ˆ5Âb¶?o^¡ãJ€Â?t
T¼u´´?­Mhß*?…,±^¾C ?ïæ>+šôŸ?UØ*ۗ1?C@X¢5?3¶6¦²'?dñϜP$P?RPü^AGN4FGL J0648.1+1605¿îì˜ú.Ò@9GüÀ:îÓr&ŽÀ<cp'Iü@!Cö6D5?ûËh´€?Ë5ª†ÑÀÒ?ÃKé¸jë?÷!iÝl@š£Š3J/?æÌ0$ŠùÄ¿ïžQYŽç?ïþ"Õ½6W¿à•NEÞ0¢¿ç榒¦`¿	ã‡AGNbcu3FGL J0648.1+16061RXS J064814.1+160708?î/ݤq ?žA>øw?[éI5Ð/Ñ?Mg8Þcp?¬"ÛnŽé?û"°ü?ç/|c—˜Ò?Àšõus°¸?‰Ê:ËE0?ŒÒ†κ?ÐÒµg‰Ó?¿÷=Â5ø"?툓^/úÞ?šA†üì¡À?t*Ãâ">©?kE(Õi"û?²x¸Ðîã?™ªúÛwZ?ìfÆ	RþÄ?˜ÇQ+Ïc@?wÇ¢"F?fžF…/µ?»M_Œá?˜LAYä
`?êê»Ãâ²?¶¬Û)º?sæwN²U?g8vLæ?õà#c(ç?¶j†¼\?Þ³=a+áR?ÇÉíîÊ<h?T©lÎÉø?—£w´"û?à#¼ç?Ç/(CjÚ?éšÂ¶?äê?ªWa!ïC8?"OCùkÊ?z üü̹?ÈS`1:þ?©Âí5Y|?ç?J§²Ð¼?°À&04]ý?"÷¤X(O?3·¸I¥>?ÐÙ²jî,æ?° 3(®MIXED4FGL J0648.2+1745¿Õ
ÊJˆÜª@MþûôÅÀ:ð‰¹QÅÅÀ<]vâµl^@ ݁ñ\N5@¼râv?Á=èƒažÖ¿´Ã$¹ô?òÛ>µGu
@1ùeÜþž?luS¿ç
'àÂÍð¿çeþj~¤¿ÛA"YÁg¿àyVbã$'¿å®éŒöóèAGNbcu3FGL J0647.8+1751GB6 J0648+1749?íz{ó&¹ä?Á|c''Á?f+,*·?eÿ6ׯ‹=?³zÇ}ÚÈ?ÁV¯ÓÜzY?åw P‹?Ãý'¿Ëª?Œà'#ä?'·˜œ¿Iõ?Ôð쀋"?ÃQ"'
¼?픹kØ&ƒ?šèÙâxÊ[?sôÇ:X?Ù?k¼Ôuûì?²è/F%?š ×k§?íæ]—ŠË ?'-JTÑ­K?y13½Î?_Ók.B¥?®t&K3?'hd…u&F?ê‡V'¼c?À¨'"mý"?w3Ð;h7?hä®ùѵc?Å*$"Ámk?ÀšL3J?Ùí­/×Ñ?ÄJcÏ:îÇ?'5@ºÁm¯?˜ÁÍU¸ã?âb>l*?āÆ'õ'?ê;
ºT`?§ì¹–Ù¸?}1
$?p°«C¼¢?ÅûØÄãÛm?§tÓ©šI–?èãG=f'?©¹eÙ!±?–("³UÌ?…¨s×17'?É°Ýù¾?ª¾Éö'iMIXED4FGL J0648.4-1743¿åNÓ¿§—«À!=‡rO¨µÀ8:êh¿;À;7SåZbL@ªšhÌr4@í"Zm3à?¥Ñl»?Ào>|<'@ãxt†@*‰
tx¿×Uˆà%¿â×nc¨¿åîŸ	›	¿æîQ Ü"¿ë1ÓíR~R¿æ"% ËÒ|AGNfsrq3FGL J0648.8-1740TXS 0646-176?ïdà²æO?—‹õ"5‹&?y'ÿÌZ?'ìN)	?–0C>Ä?‰œâ*U^Ä?õ'ùˆ?'ýx6(£;?Cw6¾wÂé?b‹H ì»Ö?ˆYSÊ¡\?ýʽö<ª?ïKч&›?‹š´i5?€Ÿ¤«T?†Ýw'b£?ØyJ¼?‡—¹Ÿ½Wá?ïã'EêðÏ?S$±·›)?.Rï¡T´Ù?(¡€4 ?j˜‹'û?RL'Šjnâ?îu§Óv¾?šb/
ùV²?{»'ÈAø?zÑæxU¸U?¥8sEê<l?˜2ŒÁ°>@?î÷ÿ^«˜0?¯Ls_Ãëð?P97ZË?nm鼐"?Ÿü|<{@?®~aŒ[R?îí
&Ú	?–x†]Ðá?ˆTkì ?Œ!Þï[j?–2HÙ`ú"?'zš¤&RŠ?ï«_cV«L?sï‰ 3×?GDB"š?;?
ÿ"å?ƒ³ã1n%?r…Ωa¹AGN4FGL J0648.4-6941¿èbI!ÆFÀ9'h›Œ¹À;×5>¦À<üF€íÑ)@!M˜.‹?ü°åEi–?Óñž"S"?ÂwOWV(+?òeR…?ù(Øç7\8¿ïÑ£Ì"'â?ÊUÆ[ªq?ïՄ̂úò¿å']džg¿·ò'ÿNTL¿âù¡A-ǹAGNbcu1RXS J064850.3-694519?ï…we^ í?°d¯i"H?C¹+˜0õ?hQ¼…¶É?f"ü¯e?¯N¿*-?ÈDÛZ?†0¨×^§ÿ?`V9ÒÇ~?jB?HGõì?†xYu?²?v3,º¢?ï,ÖO
2?†¸€€óú?i-w{ÇT?púÊ@us?—WöB.Q6?"Þ›Q5Äá?îÜ^;ZÛ)?':¿Ã'?X=$ŧŽ?RpC¿ß\Ô?¡x3#‹"ó?'9ÿ(2Z?ïŽÀ•ö'?ƒ`·
"Úª?PˆýÌÀT?GEÉ ~x?ŠiÃÓ¾?'½ÿ·&8¡?îêÀ̟''?Ÿï'šo?p}Á+ðÒó?~ì0ï¦áj?žˆv&dþ
?šûn×ÁJø?î"ÚÄBuØ?'Û±¡`(?m2KÓÒHa?kc—m/.r?¤ï/³#ý?"ļá\?ì×΢SÁ7?¡¥÷t5ôé?c['£,>?dóC,p8‡?¸¦®ÖYÍÙ?¡›®9ùFAGN4FGL J0648.7+1516¿ßz0GÆh/@KÆ!·à¬À8Û
LŠNÀ;ž¡[.ú¿@!³R)˜?ú¿gJ¹?¨Ã¤¯ø*Ê?¡œbY¯ý?÷¢™Øƒº4@ ΁­¿–?íók›Æp?¯H\æ
¿ÙςŸ,*«¿Ñâ"~ea¿ÚfÝD>He¿ÚI"ÇȁAGNbll3FGL J0648.8+1516RX J0648.7+1516?ïpvÀÚ-ç?…-)?£á?<=ZìD?0'˜?VZ¦?'"éß¹+?"ëjx˜ê?î#Í6v?¯.o<z³?[}*'˜¦?iÅ‡–K?¬çC@}Ó?®"nÌ&äº?îƒ)S+	?˜@XÙ·¡)?k¾{'©?sŸC–"Ì?¦‰ðM=G?—¢è%Ó*?îWÂÏrïa?ƒ'dâoÛ·?t¤Š¹®ï6?TÇ^øy?§ïA­#®?'|[5ÔÏÛ?î*ҟ¹]?¤8ƒYåx?Pjä.yT?EëP"Qæ¬?¬Û«²¬Ø>?¤ïß:Qy?êÀZùpð?ÂFÕS¦g«?qýqé©3?ÔNE1?Än¬Ü7?ÁÆôS7ú?íMô½à(}?£Ìâ·¾Ê`?m\;£26?q<Äé•æ ?´¥x9S‡?£a&õ¹à?ìQ£ "_?›ïg7Žæ?†ˆŸ•>è‰?n®©o©Fè?º¡Ïx?š&©íiAGN4FGL J0649.3+2230¿åCLâB,@#<yÔØ4	À;&oþDÀ<~+qÒ
@ ×´?˜?þ·.ÕÖ`Ê?É¡Ä
†k¿?œ?÷Wó?Ì6sCš@8Jaοï{KeY -?ïþ"åÞÊ¿Ýû'¾Šêª¿á$"…|+¿ç…Õ"ܤ¿ÉýC¸¨AGNbcuGB6 J0649+2228?ï!Íý›Ä?"Bw‹d¾?IV·©Ùû??ED©lC'?›0}q%ú?"p}™óW?î0Ôý®þ?­êofhŠp?\Ê^ñø_?dÂKs¼%?¬_ù~ ^?­K´ÖÇ?íðWo8Ù!?™Càðê:?r@ƁŸ ñ?i¼ƒ´Fð?®²p=öGÕ?˜WPÁ0ô?ï+Å
y<?tʞä8]?fe*¿+?H‰'hÝ?—µ|ŠPa¨?tÛ\ƒâ*?íð}0'SØ?£'ÏD6­?a}NÐi°?Vҍ^«d¦?¯à&sUd?£WÊd‡?êÄ^¾/?ÄË$itkj?pãCá-l?ƒQ«ôµ?ÄhpeÝnI?ÄuCa\D?ë+Äv^x?§)Ýq{;Œ?tîp^Øk?v¤ºÚeøg?ÂtŽŒ?¦Y{*ŽY?íʙ¶lZ"?ilX­f?x#php?gñ Û#?°# 10?Ê!F­«£AGN4FGL J0649.5-3139¿í¿ïY>µÀ,k-M@$³À9þˆˆ˜ÀÀ<!V˜"	]@!«ÝˆÜ²ô?÷½w$#Ë·?Á=wš@]"?Ĩԟÿå(@©)Äõg÷@	«èCZH¿ç¼ dŽõÒ¿éÛiQ;¿ß[™C]wÕ¿·ùl'ûDÚ¿×ÙÖà÷Ò	¿Õ^ŠD<
AGNbll3FGL J0649.6-3138NVSS J064933-313917?ïåðÑ( ?p‹C˜@¶!?>»ã¦?EgÊE͜Ë?fN×#sê·?ldRì.ç?ïŹ'ö¶?‹ˆ°ŽÞú?C'³]‰½?Q¬€ì‹á?{'A'?Š,»\ÓcÁ?fà‰Ã?™sûôYc?X>—pA­?Z
—‡Y?¥µ$ÖÍLg?™¨‡¦°Œ?î—Òâ?€ÖVÖ~æá?Y'i¤¢?CŽÃHSú?¥¶>"0N?€·÷£q&?ïÍ9¹Vš¹?{!ëßúãt?Rh¶÷õ,?R
ôJmI?tâ	6î;?xNúk¶A?ïV°áèE'?¢Yž0F»?Y
+ÞóCn?h›lP·Þ?"™A	SžŠ?¢
X۝Ñá?íjCiŠ`?¤ðö	͂?goëcÓq|?pngš£š?³òe]ˆän?£ü.Ò4òy?ìu¾1"? ykÔâ?pEUĵ€›?b…n9ÿ‹'?¾ßü²÷U?Ÿµ,û">AGN4FGL J0650.2-1636?¸yQD1CÀî軶$À9"†AΩÀ;s•}@'/bn4;@¿~/°È?´…¢ì©Œ?¨›'Ÿgu?ò=ÂÙ.@
ï+E((=?ïèsAI¿à?Ä UàÝ¿éAΡ¹"̿塏Òpz¼¿ìÁr%·¿àÐ%FáeáAGNbcu3FGL J0650.4-1636PKS 0648-16?ïMÄÀ&?§méË1Øo?vã}`!œ?¡yåi
Ñ?–hzüÝ?ž
ï= X ?íý¢A!Í?ª4Âî;WP?T‰ðc'½?`
×jõÁ2?¯Œh Ö¹?©Â_®¸Ðò?îà( Ch?ÿ¥ÇbE>?|+
?«?€ÑXšÇ?œö¡=šØ?Œ(_MK?ïéhäÅè?sî:£œ6?tŽ
Ãó?R"V‡ÍɊ?šPZéä?r{6ö?ò?íècì»?¤Øºa}Wö?n_/Co*'?l
QÉ;"Ì?¯"ÎI;«?¤><ʸTÙ?ë 3êÆ»n?À€ß?hj͔K
´?z›slRg?Ã…ëÜ?¿·°Ó>xX?î~\b?•¦:©ÙŠ?ˆï[¿"¿â?‰|;ŽEÌ?©S&="î?™_êépÜ?íGNùëÇl?'gÙ2TÉ­?›"Ûey©?t	ÔýŒJ?±ž¦÷¢¤µ?Ž!/¶¸¦AGN4FGL J0650.5-2851?ïCóÑ.ÂqÀ)ÌE˼+•À:³D…klÀ<7äæŸê@¨Ïqí®@¯äë8?Ïœí¡ƒÚ?ÙX«þ +ï@$ÚZT	m@
™á*Qã"¿Î) zb¿æ}ÿ	_û¿è@›f"sÈ¿åýŒBn¦¿ïüA&PÍ¿ðAGNbcuPMN J0650-2849?ïô
€ÇÉ?Jå=ëö?EU.è¼]ß?>ir}5?JtÎuœò??Öj=â?îZVu'Ž?³ÜaúÊÈ?€j›!'¼?‡Xgï)Mi?¦?ñÞY[?²+0¾õÛ?áõ˜?"ځ³wOé?ã«WÿgÌ?‹Sº—_?™kõV	Ë&?0cÄ!aâ?îÞíÚ??wA(HYo7?…=ÐÀÙA?cudäs™?™ž%Íøy?t§¼F?ïê?8-]?a½øO…Äé?T*âÒ~¯·?XM©N–´?WWO3O?RUôFBÿ?ì©Ì~/Ó?½uK}ú#?—ü¨Ž}Q}?¥[ºð^?´²u~·_
?¸Ó¿Có?îT´³Yñ?˜5ðŒK{Ÿ?õ…õð)?Š_`ˆã?¢ì÷j©Bä?"U1çú"?ìF*x=m8?™ŽÕf¡?¡rø‡E%?†«RŸLE…?µ/ù–$1?•z䖥ÆAGN4FGL J0650.7+2503¿ËÍXÁjÍ@&áõ±ÈÀ7ËUúÞXÀ;$ö%‹«@U)[™ñ?úãEš>H?›QZ™1G~?Hõ<WŸ#@m|²F@~Ÿvþ9¿"Ô#ƒ<àÜ¿È"HJ¸á¿Ûúœ~Pg÷¿Ô'")Dó¿ÞÇýM´¿ÈJì¢ÖWAGNbll3FGL J0650.7+25031ES 0647+250?ïî0aòŽR?RŒ×Ëú±	?!cÙ9ç?!!PÁ÷?`¹`;X‹|?Q×4JX•x?ïÒ{ÕZÝ>?€Elî[?@´pWÜ2Â?N!+!R…?t«‡; Ð}?~S×æ?î¨M†=Ò?š=Ï@è?q\ŘC	í?|՟ŇÓ?£OŽä'ø£?™›>>¼ï®?ïÖgZ­³?^M"/k?&1¼<Tˆ?"Ï7[AS?tÄÔg?9?^°Šyþ?ï֍…0£X?j1 G›è"?0ƒÝi'ó‹?%©ß2nQ?s°ÿuñ:Â?i|ÄÈ۟M?ïŠü'is®?"¡Òðt¿?_‡–h]ö¤?€Ì¾ÞBX$?‰Oì‹àÇ¡?'gÇf:Úb?î"HŽ†p?š¡6õI=˜?nÎ~ÜáŽA?xøÿ‡fg?¥Î(S:£?™Ì{8óv?ï¶#æŸÖ?rÁyb©¢?2Ü®MÚ?#æÏb{ùD?æo^ÕFó?rS͇AGN4FGL J0651.0+4013?ïÿÿ£¡@1Å!Ý À9ÖâӟNåÀ<Q¹¾Ó@J
ÒüfÃ@?¦›à›·?µc¢áy­?­âDc\œ?öf
{ÅÕ@ë÷/ü¿ÞÎAìßg¿à>ÌÄiQ¿à1ZJÏ1+¿àõ·§¡š¿â¡5íËJ¿çÒtvÊa¹AGNbcu3FGL J0651.3+4014RX J0651.0+4013?ï×+"ô%?xL°Ã8ò¸?J]YëG¡?EFŸ"ÿ?q'z‰
¦?vyb€twÖ?ïʽÜw˜F?wó«,ÄÒ(?U+°ñ³—?`ÆB<b?uV%§Š˜'?rë²³¡y?ïU^ºJ"?‰çÕºý¯}?xô_£'±¦?'±3:&Xæ?Ž%xuâ¤2?'k›Ó/eg?ïoɑȯ?g#ÿÄßÙ?s¦ù¬Ôµ?P^§¨÷GŒ?Šk,uÙë?d5XƒM?﫺¿d?wwÀ>ë–p?_Tè÷
/Ä?YKLSrE?Q´!36?sg£4Èh ?ïa€ÿL"q?'>ÿ®Ç4?jleI~û¾?xI±A
?'Srfün?Œ#*Aæã?îúQÜ&î?‰ä¼h⨽?xÈ`«B
?zŠWj¤&?šƒÄbs|I?…[ÁœÂîÓ?îž>À?ƒoæ	ç6ê?‡'ÐìNï¾?k¢+‡v? :GÙÆJ÷?€Ã¿.<øAGN4FGL J0651.4+6525?é%¡XfÑ@8ñ"<:CÀ:Zys‰d˜À<²®{¨íÊ@©µß†?þ±fYÑ,®?¿S>ìNó-?Ãb;ÉÚª@qÕ"äF@CP³¡­¿Ý
™E彿ãvõÊò×ù¿×L*ZÇvͿڝDÿŽk¿é
jKÎ4¬¿ïÈ<¿2ÛAGNbcu3FGL J0650.9+6524NVSS J065125+652458?ïÂMó(O?t'áy\®?qn=±¡ù?o™•ä•'¿?jՑl!"ì?_ÐÑ;3ï.?ï§#}ç)?'²å#¿z?dÙC®xŸ^?n`ñ£™Q?Ϥë¡Â?y|ž&Hï?ïtÌi¿P&?€sM[#Ñd?p·¿K?s_JöêG?Š¾‰ûÝT±?x5‡Ê"á?ï?––¸qT?q‰gÉóŸ?""1ÚõWÑ?b2¹Ý/?‹‡(eÀGZ?i'¦÷Ø>?ï=ã:wu?"&Ÿüàö?•Ò7Ôëp?'.Æs¹¢?€Œ\Ä Ò?qŠÆÃJyj?ï‰eU?™Z'Ãr£?zkü¤í?ƒžE7†ç?˜œ"I¦É?"ߟ탗?î¯Às¼Ô÷?"d£~ÛäS?ˆùäiì€?Š¢â,UT?ŠÿU"¸ã?Šowå[Ï?î1'yˆ?ŠÅê0ß?—Y¾i0?}ßõ¬öê?¡CV0Ã?ƒL‹[=AGN4FGL J0651.5+7956¿äªjÍ(g@:®ÿ:Þ"`À;/Nbc¢gÀ<šz¿ÖD@ÌvŒyK@¶ÌD琝?À0D
û¿Äà7bÂÂÞ@¿*?nªÙ?ñÕ;0W·¿ì/AT©P¿És—ý7MÊ¿àQ½e¿ê˜YþyC¿Æ)£L¿ðAGNbcuWN B0643.2+7959?ì¨36§ö˜?ÉÁšg}pL?µ|"s‡%?È`S8;?•	^œâ\?³AËܟÄ$?í§âõ$§!?¼­éÈ0/ô?¢Zçœr<?µ?c÷F)?£&è穽?¨óvÖ\SÏ?ëÃqÊÄ1?¨"õn@JT?±èÿ@ÿD?¢çL ‡7?¯öåCùðk?žžõ¶íÈ?í¼rÉÃ?˜¾ÜÞز?"ÚµÓ	Ž?Œ­d]¿Ò'?©fãL¶ª?'8ƒÌu0{?íÍ?ö‡}°?¹$
ï![?­³o
Y/?¸-`C¡:Y?…âFV‡"`?›
î*…¸?éO§Ñr	?ʕÝPÂT?¾AÐëüy?ÆD6™LË=?·@ðŠª?³ìSðS?éøžéúØ?®}®48õH?º:‡›ÄJ?ª+µ¾ÒÞì?¶²¬–ö?¡œµS.\?ç™é_ƒ?·ªŽªv?³4õ1G?¯¼KkÖkF?È
À	<a'?²¼c¿ø;AGN4FGL J0652.1-4813?îýŠÍMüÀ3ÃäÿÉy[À;	¼AdNÀ<³""Æ@ 4'éª?þiÀ=rQV?ÎÜ垪Ð?Àÿ±%§Yv?ñð*Ÿæ»@Z²~?ï'usI£¸¿égý	«zm¿Þ?M]Uñy¿áïç"7Ý¿ßPcÛÅ¿ãΰœë]²AGNbcu3FGL J0652.0-48081RXS J065201.0-480858?ïì^Ûáj?Q'²\LžÍ?+èb£Ì°?¤d–?aâÕ¤ë?PÓp¥Èê?ï²ÿ (‹Ý?}ª"¬"ùr?Tgúç ã?Z*/ët?€³8"* ¼?yaà´"v?ïy»'ÕIJ?x\Šo–Œ?a¾©ú2H?k'«FÊÕ?!q1ì?sf)­µô±?ïb`ã£0¥?lú·˷è?^x²"0¿??Š}Ý$ƒ?'ÌXhî_?l4ª³È›ò?ïÑ —áCã?mJØiV¼j?B…÷Lélà?6emã§?uõF½ ?l*ƒýG3[?ïEMNN?'"ës¦ÌÐ?aëå	<Æ?jœÖN¦:?•"q¦¸?'¨ŒƝ?ïPٝ{ã?…ö·6Ÿ‹?ditÈßÄU?d×äð:~A?›ˆ¶/lù)?"¡´á—¶Ë?î-ùÃ%E?‰äÂݖ»Ç?p¹zYS<?`bh>PO?«	4`Ò?‰à}‡(ùAGN4FGL J0652.5+1932?çÁTœm.@"	j­À:€ÈlüÀ<&D‰œÌT@jßÃ@zÓ}Àõÿ?פ˜Æ5?ߊë¡#P½@¡~4¹E1@ñ'1ó9?ïû	öùÇ?ĐK<>u¿âÛYWŠ¿ë¶¹ÐpÆ<¿ïւäY±¿ïÿ§ëkôEAGNbcuMG2 J065230+1934?ãe¶K1?¿zR½£JY?£Æƒ€ª>À?žÉ—Ñ's?ׄd#ý…?¾ÉXEˆÂ©?ã)ý8
Đ?ÈfBv"~I?½Göí:^(?´¡¥¿³?ÒZԛßU?ÃÞ\Õv?éŸg¨Ÿ‹?ªö©ñì?±$‰Οé?™àª¶]°Æ?Ã=¡v1à?¦Þòë>?è÷ÉEnŸ?Ÿ'Þïƒì?¸±Ï'gor?™gš4#g?¿èžm•?"çOMþ¸?Õ¥èÆÂ5‰?ÀS¬d*?³=»Ïð?ªúŠ›áË?â¼ãå[þ?ÁeÀË·?ØyN>Á´?̏dr¬?ÇéØöº÷?ÂÇߪA~ó?ۑų0¢?Ê#
Õq?ãÝ9®bè?³¢ßÛ?¾‹ª`ÄÄs?¤µ¬øy¬?Т¢®	?°«
çø‹è?ãöÈk¿Õ?®ç|C@ï?¿\ÙeG¿?®_=‰Yx?Ð;O3;c%?ªXŒÔ-1MIXED4FGL J0653.6+1636¿íÀd^ßÍ@Û2‹m†ìÀ:(°ÿèÀ<7ÚH¶R7@–¼f@kÈ:–ÔÃ?¼= IŒ¿5óT|'Q@äO¤XŠ¿ã"¿"g¿æ(þ¦ä†¿ä_¯""e¿ã³Š§ß­¿áa{_ò®ß¿Ýé¯Ü|SAGNbcu2MASX J06533986+1636432?îØÙFÇ~s?'[ѲƮ~?e£öWö70?S¯3B¥Q–?¡,0ZqÙ?ÊøL²&?ìhlw;dŸ?µ{9$Úm?gLu¢
*Í?mÇqCé&³?¼8˜¼"³?µ½]:?î­pÞ¡?"˜ûE"wc?y-͝%?o1tfŒ?«¯oH&#D?"Òh·cˆ?ï;
¯b{?pAÅ¿‰º¡?cØ^W¤ƒº?C=Z !ž²?–#>H±?o‰Ñ¾æ½‰?ì(1.mž?°oµ"¬ÀL?€³'õXÛ?nӃ‡ÍÖð?¼¼`¥"?°
õ6?çh厲g?ÆÌ´ay 3?{‡MÄ0z?ˆÝOªKéD?ÐÀ« e?Ægû192ý?ë ®r2'?¤vŎ|öo?‹
Ø~Þa³?|I0êl?ÁÎ×¼È{b?£>zj"ŠN?íº¬÷ob¹?'Rá¿Ç,"?{½øn Ò?d&Ácû»—?°nÇVª×f?ýªçÔøÜAGN4FGL J0653.7+2815?ãCïX'é&@)ÚÑÐAÌSÀ:7zÀ~hÀ<U	Ĥà@G_ÏÉVv?üê"Ash?¾È"™"‰?Ðk/coæî@®þ#†î@#óï{x¿èÉà>¿j?°r@þç•ë¿Ò¾¶4žm¿Ø'=4p¿çä&Eüd¿ïþΈ°=AGNbll3FGL J0653.6+2817GB6 J0653+2816?î*öê"ÃR? :ž§x?¢'[^`ã?™|{üzº[?•|kè.È­?‡ë²AægC?íåy(

?¯ÁZ€c™?•t5ìQö?šÔÓÜ€?¦ô=vz}?§»¥)'?ëʧÅr]?§ÄÊT4{+?µƒg¶Wn?¤wò§?¨N·¸²qS?•b†H^1œ?ìþµ!Vß,?ˆt¾Ö°t~? Ÿ±¢Ú?y6âԙÊ?¯tüF"6?b žq?êů¢›?¹Žcc/Wå?¿š,»c?µŒy'
?¯†±£"?¢ÌºªÌ¡ù?éÁ'W"H!?ÁÜÔ§3?²EeÌ?µFu
'?¿®lå[Žò?¸é †Œ?ç'pœþ±?²"ðh~Ï?Ç+¡àK@?°ë<$x¤9?µ𺁊s? éê@°\D?餡S¼–?ž¾ð³£?°oåz1Ž1?ï!šá@˜?Á5‡òäIÒ?˜ì¨(`mêAGN4FGL J0654.0-4152?íÃ=VøŠ@À1BjDAxpÀ;%ð†æ8¯À<"ľá@ ´£¶(@å¹}d¯­?ÄóSIS0¿¦	6õh?ãC
€òç@ƒ		i
?ïcÐT@Éõ¿åÖCŒ¿è"Î1&¿Ó–[@î\¿¿á¦R_Hdô¿×V%Pœ{AGNbcuLEDA 571171?ïë¶\rò'?Q•U7Ðþ?4)'TÀ>?!6Ý2r¸?aȞW­Â?Pu
Âçð?ï»æø$È?€¼ý·$i?PD¦T{?Tù=öàŽ?~lˆ÷°Z6?}_˜«*æ1?ï†ífí—??r6¥x|?\«Ÿ"Ì*±?V!KŽý"ÿ?Š¯2J9ï?p^KØû2?ï'›f€ñ?gÓ͞	:?Tل1«?6É4‹­?‰7çaAœ?gjæB´™q?ïßnÄ'»?_­P›¦÷•?@ãÁ¯¹Ó•?1¬è¦bµ}?lXKc0G
?]š,<M&?ïZä¶58?"UÓ8z.•?VòNÃZÔ?bØ-ôå?"AÚ Ø[?"Ùw·¾?ï0<™õp@?
2#ŒÎº?dë]v?\‹JÅ}3?—h/E;>2?SÊM€?îO‰e?‡œÇØc‡?pK,ÀO«?]÷÷®ò}?¥(¥'y®z?†‡ZåšG@AGN4FGL J0654.3+0923¿èét$Y@—ÊÂ0'˜À:¹C•%À<:̂úñ£@ 	Ip·M4@Úÿ•võ?Ä2T"Œó?'NÓLè?ÐA
œÛ¾@"²4°·?îQ.ƼèS?¡êˆtƒ4¨¿å
!AN¿â£¹þ"ï6¿ÚG5ß
&¿æ˜ˆAØg‹AGNbcu3FGL J0654.5+0926GB6 J0654+0925?í˜Ñ–œJ_?¾+…ké¼?2G­#?¿Iy¬?§ÙÃx}‰?–X?Æd?êHcJ?º^¯+íS?rÂRó/sž?z•ÜB-‰?ÇIxHTò:?¹¸&¼F0«?îPû'©\?•J˜×1<©?p·îM¿h?d^Ko¼'?¨ÙljÒÕÒ?"nïQ%g?ï(Âqݛ…?r5~BúFE?^Ð…þcË?B`)yd?˜ú±:à/?qïjíŽ?ë›ÒRŒƒ ?³@âS<î?'²E&ð˜¦?ª
æT"?Àe'e·2?®·¿"–?ä¬`B'Rø?Ä÷ÞW}")?|žoÖul½?Œû?ÊòâH?Ö4Å»Fέ?Äq¾HÐ~]?ë‹Ö'òëÎ?¤êh\=v6?€™±e6÷?uþógúÙ?ÀÇPgÃÖ?¤Ne£#ÚE?íb·Í-½?KÑ3ï?u\B³EH?c5"¢sv?³kÓ7Êó?"GCb4»AGN4FGL J0654.3+5042¿å×%͈Î4@5ˆ‡"žÀ9qal+¢À<Ë­b@ê/o¯:k@™'¥R?¦æÏ=¦Ý?´%`Gú|@2Ÿà·ö@ð…×ÅÏ-¿Öü°?Mrпßv–_Ruï¿ãšÑ!Æ#e¿â³9žeË¿å«äT¨ÎÁ¿ïÿäQMÐmAGNfsrq3FGL J0654.4+5042GB6 J0654+5042?ïñáL.?Y7œéÎ?:Ÿås
N?-sm;ëß$?V<D'òÊ?X(!»]?ïà9"5Š?l%LéÒ?Cæ1ü®€?RØ»–b8J?jñ:_¸Oz?fèT)B+?ï«>â`TK?zG‹ä¶¼?h,5¼õ??róßQ†ö?~JsÕÞn?srÃkKÞ?ïð3?ƒ´¼?@6+p©-ß?3jÞ̔23?ôå'Zñ"?Z¾ÉËÛÌ?=g¢¸^&?ï蕾m¹?Y–È^"È?CGµÚðF?7c«¾ùK×?c§ ×Å0?VÅÄ¥Íã°?ïªÚnËåœ?ƒ¢¾Y.I?W$Þð/O?gPª~w‹ô?'dÈdYÝ?¸–$"4?ï~Ë
É°ý?'`'ƒÓ[?q¢üœ+Æ?v8"ˆ¿Çv?‡Ãk¾hÒ?{Î>`¾©Å?ïÚ8Œ¨3T?^¿IŽ?GžÿŠù?5yΒØú7?pE¸'{8?[[ó+ÀRAGN4FGL J0654.4+4514?"z—ÿCJ5@3cag#$ÈÀ8ë¤dζ²À;ԕ"´@?ƒ*+ù@vÞüz9'?§[ADT?´‹¿f\ÖE@{…L»@'M³çùy¿Üs k°R¿Úd_ó.á¿ä£PÂe?Ë¿ãHÑ?£.¿èåo®¿â	Y€ù»AGNFSRQ3FGL J0654.4+4514B3 0650+453?ïö.X`œÖ?A%~'?*Ìô¹1±?Á†«ŸQ?PI°"zc??Ž™hé1N?ïåQ¹e?m{çÈÚ?AN"úób?QÊ»‡£u'?fZþ-3ì?h0àCáO?ï²tŒÍ`ú?uf"GD?cr¸‡]ô?kûÂz®²Þ?}]7ô2?o¤QÁY?ïú!"<w?+× {Ç?zelŠyÚ>úáŸraU‡?E*e´Œ2?*p]ĶŃ?ïîBwb¦Ø?Qz:œÉ¥×?2ÕÐΕl?#xìäñ?^ÅÍßfâ?PEZã[?ï³5ƒ^]?…œ|ŸØl?R±ðl»?g?Ù¨y?€Üa|¸r?ƒ"]Rãr?ï|¤ôª¦?€µGU9…?n÷î²Opõ?qkHf‹Ñ5?‰‡#2P?zŒ>-âb?ïñ\µÒN0?JŠ
ºä?'<éܳ£?ÅúÇ›Ó?Z^÷N,0?IN6£˜¼PAGN4FGL J0654.6-4952¿Ý}ãWu)DÀ3è÷‡‹zÀ:™7ÿJÎZÀ<{OnÓr@JRÃFfA@:6\³_?Àª$@ÒA?š;aµ_?×e …±…@û7Ä<…?ïàÝÆTe¿Ž×GWµý¿é´V~'ÖW¿á	Ò¾@î¿ì˜n÷. &?ÊSØÚ¢"AGNbcuSUMSS J065518-495205?ï6FA>?'߉>·Þš?dÌđÜ`:?X6Wu!f?–ŸG4p@?'m½8SZO?﫝ćÀ?|úˆ•ÑD?]ørBÈT?bü^Ø[?~ÊFCàò?x,8ÚÊ`ì?îå/;Ìú?'F%a
i?€ùgLüÆ?€
5öAR?›J›èOöh?ŒÞ¶¤ÚNò?ïhŸüSg?jZ²dQõQ?v".ÏQ†?VÁg'a?Š–"Ã?dèØñµ?î›I¤8Ú?›Ȩ#?ã?y=ã;×M+?ncÓÉʧ?£'>ý#©>?™d–tÏtm?ï [IÛZ?–ß,·:Œ?oæ+ÏÛÚ»?'½Y9"[?—÷ÊTáÿp?",NØAr?î,4…‡'°?™o{ý–2 ?"lÈ Û;×?ƒÓy>yE8?¨!…~ã'?—
žƒR?îB¶dfÃ?†D3jùc¨?Àÿg"\ö?vôEorj?£tRK?
îà漺AGN4FGL J0654.7+4246¿ä¬Ò@2›ðgȗÀ:VÛó±=$À<XÌ'=«@ P2O2˜.?ÿ†'+½óì?¾K'Ð|°?±ôŸÏ"§?õÓ±Þ3ý^@Y?E:G?á5av<??ã+žI+Âü¿å(M[Óem¿Úà
Fe¿ä¡C§½¿ØÉB>=þ=AGNbllB3 0651+428?ïŽlC8þ"?®âGœŽœ?KÉhÛ)2×?[ªÎ3¥¯?Š¨X–r‡W?®×5³ƒ?ïÇÚîVÆ?zU¤zÝx?S£"&Yµ?]q^Šñ?w)§úsŽÄ?tՖ=¥B;?ï³£áϛè?pM
+7r?SØò÷>œ?9ô§—3Ä?€›éKÑÄ<?o¹É†7S?ïx´5•þ?qÏÖÄ~¾Ý?¬·ýáƒo?[‹Dj#o?—E»{4·i?q0˜_-?ï¸S.-îX?ƒ~FCª3?VÍCíÑn?KDý]AG¹?~#ÍH=?ƒ/ûÚ'F?ïcwŸZ?ŽSJVš©U?g©þ"6®?qb8'U}?®zvý?‰5ƒ»#?ï~7ÙU?z¿|lŒ&?\9Wku¸?Kr¿†OŸz?ŒëÓ¥Í?y ÓSu-?íDÆÐÖ¿?ŽÇeå½µ?•mÃb`A?yÙüJT<?°~X¹i='?Ž$•í"Ö©AGN4FGL J0655.4-2631?³ãç<6ÜÀ%Ý)V:Ÿ8À:u	A}À<8$â7˜@JÎãþAº@KCË0ë?ÆHÆÃHi¦?ÉÙ¨¨UI@᤽º
R@(…a8ª¿ìS^¡Ëí)?ï÷Ìàméh¿â"¤¢Œ1|¿åF–Qæ|¡¿æìãË¿ÈÈf¶˜WûAGNbcuNVSS J065523-263041?ìú
«ˆ7$?®tëžÄ.?zíûÝäQ?rù ؇ª?¶€Ò¥v>?­'\Ir‰?ï79Nøƒ?ŸDl‡
øa?f©¡
ése?qzu÷"?–C¡úÂýŒ?íâüLã?îhiéR¿k?'T—60÷@?|Fìü'»S?r_E™"÷€?¥ðƒÎ:¼é?šˆ~'ú?îgJÏ­c?x¤"†°?ˆMaýr?cœy`ÿ :?£‡ËÙ
\u?u§ç}6¾V?é'e›î¼?¼sÇùŠ?'4T®H¡[?†€©È5ÅQ?É;3ÒëIå?»EÚ©ˆê?íø"ʹ"?±ÀIÎف?ÁÖ9^ Â?'xŽ¸é5Ñ?¬=Âê\?°ÙƑfž?ëan°þ?ªpgú˜À‰?"ß«¨ŽÔ?†U3m}¢f?¿ÿùŸé"Ú?¨%9ËRÏ0?ìFN¡M?'[yj¨?šèÛ^%žL?&´
èH?¹+–´´h'?'ÞÌSAGN4FGL J0656.3-0322¿î´¶ ôþU¿Ý
ÍÞo·sÀ8S&ùz«À;‰ó3hã@ð¶ÛS@WwJº8v?­\ãã?ΔBWC@´'¾‹Áj@°'¹%{¿Å)̗Àñ¿á
Hï]¿çåàϹW¿é¤''¿ëÆ?wå¿ïÿù_|è3AGNfsrq3FGL J0656.2-0323TXS 0653-033?íÎ‹ÿ}?°ùÒ*:?¬âÐtIG?°QÉ̪L¡?ˆîüÍp‹®?'h	uH?áéd¡Pƒa?Ò,x•x"?¬õ+‰ÈJš?²ìB¦FÓ?؎'L\éª?Ð|Im˜p
?èSïx?Ï?±1óMÅ#Ä?ÂGtôɕ?«¼7Õä‹?¸ÑšTê
?¥‰'ª0~?è
B¤r?¥ÌsÑ­?¯a´È@˜?'DѾ4ç?Ǽ~‡*½T?¡yHþ7??ë˜| ?·ûéRNs?º|+Áò ?¶#¸;Ò0g?¡YEªNà?—ûE5]<Ä?Øe¯3.5?Ðçd?g…?¹`ƒ7'jš?À%-ÛIV?à¡ÿ>þ²?ÑLü ­'¨?æzÞã;í?±ôdP5'?ȗã¾ßW?°H·Gã?ºúÑ aè?¥Ï.+*ˆç?ÜHy'ր!?°­ë†or?Ä98#­%?¥C*MQ/?ٚêÇ´Š?°u5ƒIdMIXED4FGL J0656.3+4235¿Ø_‹¼óL@2Ó~=ÁÀ:³pޏmÀ<P%üu@ Ë­R3(¡?ÿyó$÷0?Æ>oçÄtå?º¬³æ?÷5'm,S@œèwx1•?ïù-Œ*E¿åùy¾‡å'¿Ñâ<xm¿áÄcq¿`¿æ"À%?nçcsdH AGNbll3FGL J0656.4+42324C +42.22?勇û²Ç?…Ò¾©HŽ9?TÖ¨¦Ñ]O?L–3s¢÷€?z½<_L"?"±+AýD?ï1ä\>"?—l"5úÐÑ?yÉáP?xòý9MÜ?—sÐýÌ©?"<Ë>˜œ?ïQÿ¡MÝ?'dÞ¤'*8?`îþùaT«?Vd HIlÉ?"¢?,&(Ó?¾ƒ
?íÒ Ò;)?Œº2@o?'¾Ã–`ˆ»?bD×@àB?°¹–‡gÿ?Œ$,ñܙ?î»ÃçE%?›¥dMé_?eA*íìcŠ?Uƒ&V|®?¢ï®à8ö}?š‰ZŸBVæ?íâß²œc½?©ŠJFJ<9?‰"*?\˜?¨W(ƒ?«m:QEÔ?¦pp£¨§"?îBôഃ?—ê@o°¢?pë9"éÞ?j·Î2ßm'?©Á~?ñ¿?—
rÎ6€Ü?è"Ù:Áü?¥GuûJ]?—N=5ü¢d?€¼5k½?ËÓnýcÃ?¦1¬§AAGN4FGL J0656.3-2404¿ëËÇû#DÀ#d¶0©À;("VÀ<dYV³jü@ €õQ%aŽ@ŸKÚÉå'?ÆrÜV¿H¿ƒ¢õ
ÐY?Àh[3,}@aþÍ¥æ¿æCé>GŽ_¿äڔk\om¿èI.p•¿£ÛÔQ¦eÛ¿ëlé7fž›?ÁÂkŠg¢|AGNbllPMN J0656-2403?ë¡3ó2ÎE?¶UÂP]?u¹Þ³í?nºn%wˆÎ?ÀÍa>«®¼?µœ7ÕB?êSÆÆDê¸?»¥UOàþ?kIMœa?qê':CØ{?ÆDÁ?0?»Q&ºe'?íÊΗZÙ?š¼@͏?zÜ9æ!zÙ?x¹Vs5I?°¥ëü+Ï?™6›êÏ?îÙ2ºx‡?€ø¶"…~?d4gÜ¢H»?P²FƒXû?¡)Ü»Ç?€hÞd?çu,UYµ?Àx_0ÖÑL?:êùü
?s-'´Ê?Й	ŸC°7?À5§SÊ
?ãŽùØsŸ	?ȗ̸³mß?nTkú;{D?~uúijùï?Ø¥cvòИ?ȁbç¼ùV?ë5¦ڃ?¨\B¹ "?ƒÔwˆ&:?~ø"~k©?Áì ˜r[?§i¤³xôÑ?ì9èjÑÉÑ?ŸÇ¦Æ?¶¿Vƒû'?th.?i?»ùä¿Õ?žÌ}8é?DAGN4FGL J0658.1-5840?ÊÂñRyZÆÀ6 ÝDÀ:Ó"d®ÖÀ<šU¦$ÂW@Rmⱑ@S»¹/?Ã,hÿ?´ÂÖÿ«œQ?ðΩ+Ç?üäò7ëSÌ?捻å'6¦¿Ñݦ䱿ÛY—á]¨}¿ç¼o¢OJÁ¿æ¢nŠ!V'¿Äpêù³Š±AGNbcu3FGL J0658.3-5832PMN J0658-5840?ï±·m?¢?uC©Oí?J7¨RPgŒ?7Õ>'GÐé?îª*&e?tÁ7˜G´õ?ïs¡!1~?ƒp%‰ÖÈÄ?m§sž ?mL^òŽ†K?‹­øY.»?€5ñòª¼?ïLöìv?'Û­å$ã1?pJ®­-œZ?o³œN#ªL?'N"ÔD'?€h‡åÿ?î‰S€°"ˆ?|—¯ž8›Å?ˆvµÇ€:V?eÅ͕!ÍI?¡M…ª]é?zi0šxy?ïp9Ä¥i?Ñ
6'çê?ZŽßqŒ*?JW…‹øßE?O΅šÅO?P©çs?îy?¦"÷?ŸÊ>mwG?FY'Òáö?"nŒ®³3?¤ƒ:k7Î?œœ;¥ìë?îÐJstI‡?ŒÈŬ(*?vl" Üê?né¬Pd@? -Æ2Y?ŠØZŽZºû?ëáÐ3My?•lÃ6k?žYHæǛ?…KM¯€ùŸ?¹[,A¬'§?•j°·ãõAGN4FGL J0658.2+2709?ë_ߣí@*ÍA·ZtÁÀ;½x›óÀ<…®
iæ@M†›@ì†;?ȌÇÀ'?yuD½®¨ž?ªLõbSmw@ÄØÆU9m?ïe€Âø¹¿×Ñ}
§¿æ̝Òä>¿ÔÊ#$G]¿é"Ì«>Þ¿Ü#"$ÓAGNbcuB2 0655+27A?ïX­ªŒtÝ?ŽðñÏx"5?\x"š/ËÝ?Md̲gÀU?""Âc™­?ÿšà4–?ï¢pEy‹?¢‹Z¼?JØ©ØMQ?UÖ.ÑËÎ?…¶d*¡ê ?‹è$àí½Ÿ?ï¿™¢AÎ?Œ;uuBºI?j{}:B?k®IƒŽ?š8%K[L?Š&ŸO[Êæ?ï¼ùXyœW?Xý(·:³•?VÏ+WäÆÓ?7TáLîp?{ψýÖÕ?VÐÁ!À"‡?î@PÉW]›?£B­©=s?mè§\o~?gÙ]Ö×1?ª)Dß}W?¢É÷ÿWBð?îÿÏezÐx?¢–ž­ù¤¦?\pÏ@Z'?nö¹)ᶣ?žE¼=V¤\?¡«þl¦?î2®[¦"?4áÖk©i?wTéI¿š?uGo!kK?¬27ö'õ?›}¶ãL-:?ïB\%Å·Z?t ô	¨?m—z€Zˁ?UJ3ǯó?"‹þøÚL?s'AÞãvAGN4FGL J0658.6+0636?ëó'õCA&@j¶ÂŸLaÀ:R"ÅõB7À<+°¶ì'@ °jûw?ÿKXÃæt?Ã"ÝûsS_?¡¬ØwHP?ßmõܐ/@Ûäkyö'?ä'6ÎÉ&O¿ëów'1L¿Òˆ:̄¨¿Ú#ìnRÄ¿à¬![š[¿âžf½¤:ÝAGNbcu3FGL J0658.6+0636NVSS J065844+063711?îˆpF¹øµ?•"ýÝÎÃ@?aÄ@´?O6¨''Û?¦\·C—i?•;Ú܆?꜎QÎ?¹&eÓ'?u+nñ o?z`Ë°¹¹ÿ?ÇP2T]qÃ?¸\oÊ@À	?íóÃ&÷a?"ƒHžN?u7Ëï.ò?g—ªeø?®Ô:ï?"ØC'ÉŽù?î^Î!Ç·?†vÆîâ?rÏ˚Ä]?PïÑ­—?§ÅÙ¦j†ˆ?~he?ë÷«:Uç=?®ý7XáG?yD/÷=à?jX²"ü‰?¾²aç{¤¼?®
.?â£!M‹+Ë?ÅVO "Î?~z"(‰Ê?‰…Bl©ö?Ú?ÔÛ}Ùc?ÄÉAK"–?ê‰7[Xbº?¦'RòB?ƒjw"ò}?o÷Lž…cò?Ĥ{"äh?¥–Kªzã?ë¥u@°¦?"éóøU~Ç?…ébŽþP¢?m±D'ņÓ?À"ÓâÞ?•$k¤{»[AGN4FGL J0659.6-2742?ïÿ¿[}²¼À%/UÞXæKÀ:3Æ&À^*À<3"'ʘ@X‹®õKq@ÚíÜçÍ?Â\ÉŃ"?Ӑ{xFb»@íÅÖ8†Y@‡¹Wzf?ïû7mª¿Ü´>¥¿ç(Ãm¨z¿èjÃQ#¿éÿcøÍܗ¿ðAGNfsrqTXS 0657-276?í͕äG,?³ßå·J¼?¯;>ø?¡éëïçSî?°Uæc?¬Ö¬ñüaY?êd£½¬?Ü?ÀýÈDtEš?ŠE™ÀšŠ;?—W"úC3¤?ÄÉm|Q­?¿cÝeUÖ?ê–·f'?¬FˆÂÆ?²8YtcÊÃ?¢fv.§Ö?¹Ó6ô3?¤¹‹ów?îY¤ßÑió?}±yyc?[Äùy(?jMÒ$áE?¢7χ䦸?xÚ6ø?ëÜEA8ë•?·P3q5¡?£&¹t¢¶›?£§"pÒ¬ß?·Šy>
	†?±ír£z\×?å¯ìç@ãÂ?ÊõŠtýG?ž°Éá´0?¥@]tAžÅ?Òµ$"Ä X?ÈّÊJïñ?軕½l¹?°¾"U5·?µŽÑ'p†?£CéB\™?ÂJ@wá°V?«jÙA4?ë
èÆtæS?šw¸Tbm?¨´Š|›?Šø`š¾×?»N·"Lfœ?"y~ñø€ZAGN4FGL J0659.6-6742¿Õú
å#ŽÀ80…†"À;Z©Jç"ßÀ<¿<ÓÅåR@"0ü@ظ=?úƨZý|˜?Æuøˆ‡?œãg‡½gï?×p§\û®@á*ŽÉÝ¿ÌÁ¬­O"¿ïúeA"_%?ïú¹¤ÑÜ¿âït'ƒ¿Ü»©ú9íb¿›…
›tAGNbcu1RXS J065933.5-674356?ï×±Ñ¼?t¼ P}²?0Oe9[é?7~(8-ú´?sq"æD?sŒ~œ?ï°syÄ<?'áŸXé…?TÍM'´z ?aàU"@ђ?I†?'?/N,¡ß9?ïB^7©öš?‡Hr"#"?Vã#ۏMß?UöL¢"!?–FÊt'ß?‡ܳ··n?îèn'qò?'Y3õ¾D1?NËS삕?AXÚ
1j? üñéÍõ¨?']Oìpcè?ïŸÁ,õEV?•¡H)Üh?@÷,ˆ?J?3†,óE·?‡AëÉ~?~úòá'a?ï0%ÐQÅ"?š&«|œ¾?c#âçx,?r
‰Qÿ?—–É¡i?˜Có3Ž®Ì?î҄9©"?KzkšÇ†?Y;.dÏZï?Wk5¿¬?¢
æLȉ?|2øÈ ?ìÍÁÞÁ? ðƒSd´"?^cH*?\Î?¼)ã?¹tVRÔ? ò´1Þ:AGN4FGL J0659.9+1709¿ëS;Þe@#¥ß"9çÀ:4\|ؙÀ<‰£–@(ÄBd©x@#«äøê?Áï,ž¯N?¢_ä°Þ?ÝÛB›Ûé@
=‰T'¨¿áë5@L ¿æDI,«¿æêò®~¿çbår¶¿ë	3ðÈT˜¿ïÿHë+\¥AGNfsrq3FGL J0700.0+1709TXS 0657+172?ï'éÐ1Ü?®³×Œ³?Zá졦›?o…c,ô¬?‹é~Wu'?¬Â™aÍB?ï—ç8¨œ?"j$¿…š?H¥çσ¹?Y"éi®?ˆ{ÚDn>Ù?'^ãÀMEU?ï3éf­Ö?Š`'Báq¸?m"Fx©B?mL§œòC?•ìF­?ˆÝ¼œž?ïÃÙ¿W!?X'F™pð?LLkŒ—²Í?/¢Šáÿ?z‰'ÿaJ¤?W6à+Pþ?ï,G1Jƒe?àn«‰z?fpáÀ(€?W¯œl0 ?—¨ýv´B?Œš ¬gºj?ÿ•T™?¬,`¾Ù/Œ?aò?GE"M?~¥Û1,[?£ì?ç´?«âkqG~?î{ZÏâßf?–vêôÔH"?w0jv®l–?um:0ù€?¥dE³j/‡?"¤B?½Ò?ïR~o*¢?z6^èµå?do#~Ö8ø?Pâ†zŒW?""M±…«?xeM²@ÜAGN4FGL J0700.1-6311¿îÀ½Þ%oÀ7·ª%ÙÀ:±ñNŒU
À<˜M×ú'y@ )ƒ:1ª?ý'-ê
Ë?Ƃ_UÐìí?ã©'#V?ýÖ—Péý@ô
8"x¿ì(ǀ?ïúªùš‹¿Û["ÀĀοÚkaýËó¿äãacÈ&¿ìó)WèbAGNbcu3FGL J0700.3-6310SUMSS J065958-631238?ï·´=Άz?®Âšì@_µ?r¹,Š	G>?®•¹qBÞ?ql´§p«'?€d[4D­?ïÕ+4P'?tؑ£—N…?DÞ÷no˜6?PQx/bnÓ?rΆÓÉ·3?rV8¯hŸ¼?ûT
?sÿkÍÆ«?[À	Õ?dß¦Uo?"ŸÝ§ü¸í?q)qŠÔ&U?ïW'Oæ?l"´-"¾é?o‡:£í>?M.2FééQ?'*8E"Hw?jÊæä=;Q?ïʞÍò"?pøÀ Ù?VõuÂϓ?Mu2³J?tó;˜|Ï?mÅ[/ü?aN#¤?‹¡ÙY"0?XLK6¤÷°?hýR($b?‹Õ^Ij	è?‡ê.ŸŠ%\?ïY
Ü«¿?€¡Í¢70o?eÇ=)á?g\¹¡—h?';Kœº_?~E<ÍÌ3B?îvþ?…lj,0Å?é:w
h?eÞ)ŠÍ¬Ñ?¤¾ÂóÛœ?ƒÓÚÇ0AGN4FGL J0700.2+1304?Ùhš%äÕ@h>]2àþÀ9æGÁ_±À<(É Èb@Þcðë: ?þ«rßñm?ÀéðÊ1?¹ù]ú\'?û±ƒ›*"?ñºØ®'_?ëKg<O;§¿åj(3¦¿àà Ç`¿ÕZ¤k¿äÐeÁ•a¿Öi}±ÇAGNbll3FGL J0700.2+1304GB6 J0700+1304?¢F?š"ƒ)òk?h
ÉV#?]{ɀŽD?¦'-·æd7?™'‹V€'V?àëÉ©E¢æ?Æçªý!Ý?¯ª#3­·?§±\ÍÄ/?Ú3(G-!]?Ä30÷ø'L?í¬©Z››Á?˜ÍZk?µ—4è$¤?y‹LÑCT?°dD§¢?– Þ´Ð:?èŒù	ðo?™Î%stD?²ïÍ{õú?ŠdOÅ6Â?ÄT5:¹(D?"󌡅îŽ?ë¨Ò#EKÜ?°k¥6þ?ƒ.>À¦Â?x­ÃMV^?À)ӅpR?¯.1‰ÃkX?ÎÊIoW?ÏYF¤Ì?·(}¦?¸=W" `ž?åj×(½°Ç?ēÃN7µ?êáȀüƒŽ?¥&Î( Þ?'-Cï"Ø?@!+<zu?†k&óŽ?£ù`â?'?á'tÅc?¨Kzâ%Lá?ÀÿMÃV?ŸAË5ú·?Ô^ ‹"O?¦3DÔZMIXED4FGL J0700.5-6610?îzƽMÀ7–6—lÀ7àóÌëÖ}À;n,Ñð"@zrè)õr?ÿlV…GÒý?˜´C÷ä?³èù~0²z@H	N][%@J	99²~?¢‹>šÖ—¿Ø}å,õ,¿àŠò×ùP¹¿áQ¦ é4¿åó`	€¿å™
Æ(ÄAGNbll3FGL J0700.6-6610PKS 0700-661?ïë¤x¶S?U‡s¿þÒÀ?5ÊhG‡ß?0‡¹€õ$¹?a¢ŸyòÓ#?SGB1•/?ïÉátñæÚ?xª®uæåf?M|~7 >?Uƒ­}]ð?wlµäì'Ù?véúšÔB?ï«ÙæCsü?ƒW(Qù?eî² ¶E?tˆø"ñ?ƒiÛ-?€dfvÌy?ï·¼§2*í?béÝËÂ÷?X-ëÚñ?ACÉôàä?~1u9D?`â_ÀáX?ïã÷¸ÖF?\¤×t$£?5°§C›Äc?.Ò*K49?iR2f×gí?Z¶™ÆJ´?ïpQÞ]ݛ?"AÏO«[Z?d}t†wñY?wÒ¸fÚë?ŽÌ+Kºþ?'ÛƖ¦ê?Ðí:M?"¾±Ç=?dJ1‰ˆR?t¼õG?ƒ
?YfJ?†*ãóB?ïhؕœ£©?z‰§f¿ZQ?g(IΔÈÛ?TzO¹;‰?ÿÈ»¥ž?x±Ä€pAGN4FGL J0701.5+2511¿ì¨Jžoþ@*ˆšgó
À:ñ/¨;ôÀ<‹5RÈ$@!""«þÎ?ýïüÍE˜'?Â`#×·¿"€-Hâ$?ӋªãÃß=?ÿ8·§ ÀÀ?ç–_½Õ¹¿ë%d`ãð¿šÚ}xg¿éCN¾ÿږ?µÝ´¦M¿Û'@dtßAGNbcu1RXS J070132.1+250950?ï6uæi´'?PIËì?Lr£º?<®à?Ä8?˜PÒh]°Œ?ñ™wð-x?앚nUÉ
?»`Ž'((?Eå(—…?ˆ‰@ù?¹*oèù±»?ºçŒ8)Š?§p
Ä?'~ߌ •j?lJDʇ^?l1QÝF…?£ÑÑ@iÉ?'Ì-q{Ž?îÂø^\<þ?ƒv®wªý?V"†Ç
Qî?HI}™IT?£Ýà~,?ƒ†³ï?îLJØ@?©ã?ÙH?a=½G˜Ú?Wݳn?­Ë7¶ÐŒ?¨¾'GPü'?è'çDáö?Ê
"49?ˆÈƙ12á?•â;2«Û?Ì+ց›9ò?ɏje=`M?í	ñvWþ¢?£EÞô|+?už<'i¼?pæø©hÔ^?¶_Ji¢ßR?¢–À¡è•?ë¾Ä2Q¿?£Ü'wóHæ?o){%œ'?g{ñpû«?ÀˆIùPìà?£Û°ŸnCAGN4FGL J0701.5-4634?æGsJê#À1´ÖÂïÔ9À8ýë7ñÞÕÀ;íhò1á$@àht³†@‰bI¡3Â?©¾X»æ?Äâçxb<@4aQJ@½©›ð6¿Ì~UE¿]¿áŒ†'ø¿å‡)õœÏ¯¿ç7?#Vq¿ìíÝ|艿ãšÑ½woMAGNfsrq3FGL J0701.4-4634PKS 0700-465?ï§jß`¼ó?yF ûôÔ?wy¯Óqž?qòÙÙR$¼?tÐào!d?kTU¯ld6?ïæ\	/‰?n>	»î•¹?;ëDÌ(³?I
6í¤—G?fA9sM±b?kgûÆE®?ïÉgMÓ?"ÆÆÖòG?‰kC}ª¼?Èd"Ð9?'%°ƒ"?ŽŸqT>M?ïé9Oµ}ƒ?IënÕ[&?EÄôn¦ì?1`Œ4€"†?aUsnžƒ?Dˀt—%?ï4
ûup‰?_Øâí'?Œ#ž¨'©è?‰]8êŠ?†Ù¢‡Ï£´?\)" ª'?ï¶î!ÂX¼?ˆ$×/9D?X={[Ï\?rP_a
9?~ySŽŒ9?"øÙ¦ §?î×æ¦	6?šM=û'$¯?ŠÈžQÕ®Ê?ÒØÜMéÛ?—žÜ¦6v?"VÏÎîù?ïÀäˆo£?i*Sx"ˆµ?^¯à‡Æ?N<0ÚàŠó?wáÃèlLo?dæÒéAGN4FGL J0702.7-1951?ë4¯ÜÉfˆÀ_9K{)À8°µ "µÀ;q׉¿1@êwY¨½Ï@ ºK?©ôr-Dé?¶Í´~La-@
ۇz³%@b
Ë5¿ÐìK¢ë§Ù¿àÏ9#7<­¿ÞÕPߖ~¿àèuÕo2¾¿å,‡m¹—¿æ¢Òþ?5 AGNbll3FGL J0702.7-1952TXS 0700-197?ïÊ'iYž?e.—¼ Œz?8JÌ܁ô?+*´'‡šÎ?ygž®Üç?dh»os% ?ï#"`¹m
? W#muZ?A¸wƒãU?RVª2ÐV)?šÿ°,‹¬Ð? 
f.­ô?ïv'úùcŒ?}è-Åó?dÆÚ͜ý'?j´
dŸÃQ?DJ†͕?~˜
âKÑ?ï¶|vÑ¡&?avWðãʙ?CƒpüT?)-u"±êu?(«<Pµœ?`¬ß&U§?ï‹TÁg,Ï?€l'ºõ2?B7TxŒo%?6ün‹p?ŒZY–3?€}Œ¯µ?íƲóCc?³Bs}Ê1ò?Wc€p^[?sݽy_?±lÚd^%/?³wýB?ï%²T"]?¨,­¨²K?k÷¡UvZ?p"¬ç÷m?—ÊÁL"?ŽP@XauN?ï_ŠõÅr?xŠzIñ?TÕÿÜǞ?AŸ¿¯0ˆ?'ÁAEž†?w"%츢aAGN4FGL J0703.2+6809¿î×®pHðè@:.Y¯ž¿À;Äp/=mÀ=y@]¾!@!m›
à?þÁX$"D?Í¿9?«BNâ™ÆC?ß:#<p@#_•'Í¿é(Qû,Ý¿ìÎÛÐuι¿¦èsFs­¿Ý»ˆÂ0ç~¿èóá
Ìq?Øߓ£áF,AGNbcuGB6 J0703+6808?ïÇØ+z­?"ËkxÉëF?3|8Çcâs?<—W '5?zÜ&—#‰¦?"ô3³×?ï"bЯ°\?‡3‰˜GE?`8ø¥[ÚG?eÀLêG?†Ù
¡
g?ƒûDdæ?ïb¶û̌?Ž×Vµæ£°?_*|P>¤?f´¥R!B?šÁYʶB?ŽT÷ÉÒ&?例ä?jÁì˜ré´?G«—vkö?2¡Tz]ð?"ØŒ¬‰&?jÔãa+ƅ?ïooÜܺV?'±–O)Œ?@¨kBLŸ?2²J¬9~•?'ŒÁ¹úª?'›Âÿô‹e?îøbQÙ¼t?£CÒ¡NÏ?i(¤‹Ónæ?y¥•¬N¥?Î¡/²lœ?¢ÀX™Jõ?î'ˆ—`%Ò?™¯§;Ýj™?g^:»Å?ô?iÍ4­"þš?¬'Ý9lã?™÷«6"Õ?î³c$'†?ŒÔÎ+¥'ö?^½~d*À'?Rԁÿ…³?£Ù
ÜcM?Œú/bl|mAGN4FGL J0703.2-3914?»L*%'—À-J×ùP¹VÀ9Àø£lŸÀ<6¦CÌ«@b'vŠv@|_ag?´ÂüÿÅr?°uŽbÿd?ûBJÈ{.u@Q&úë™?ïñöó4¿ãå"~°	H¿â´½ý&¿×ÇÚñR¾¿ç$¢¬gÒw¿ß	žs`AGNbll3FGL J0703.4-39141RXS J070312.7-391417?ï¼"élžA?r>}#	´?PB½%™›?A´½j‡+?}ÝÜ®l?pî"7+s?ï¦pÜOæa?'AËm¤c?`'™ÒNîÝ?dמïè?'?"€a§ù?~"ˆ?Ff?ïEM²²½?ƒI¸Œ¦?nêöù?jqly‡?"ÙrÙõ?€·PnŠ£?	^¬?uÊ"
™?ŠÜ¹opýÎ?bõùµÆÈg? 1
ÉcŠ?q‰nRŒ?ïg9'$?'ñæÏÜ?jËDûÊI?^‡s 
tí?«™öJo?৵½ñ?ï	QÊô‰?›Thüð`?t!–M=Ü>?{OìC¸ü?™Ía#.Îã?˜êýkNxK?îbÕe€@
?"£ýzÞ{?€1oÀ€ƒá?z‰ǯ "?¥ÆM¶$l?'²dõ×?ìI°˜c¹Ž?'Í¢@ÏV?¢?8äÚä?'2Å
‰€?´'ÞÈÛx"?Œ)çÖGÞAGN4FGL J0703.3-1042¿ç=¡>\9ÅÀ'D`'!À9j‰r¡À;HlÞO¬@¶6]_,@5£]gº#?»€;"n?"‰y­ò?ÙSËäÅfý?õ˲BÝË"?ïìfZ§ìC¿»ª¾–9y¿ë0Ď9ê¿é;(àsó˜¿Þo+|/¦a¿Ô‡B^Ê:ÌAGNbcu3FGL J0704.1-1043NVSS J070322-104426?ß7Չ´Ê"?Å8
ør6?s(µÄ	?júÜö¿y?à=ÃЭ_¨?ÅB{vT+b?ã¶÷áßj?ÂUÀÇ¯?†µ…!VU¼?†sÆ¡Ø?×Üe¥ºþÞ?Â@°
=D?âDƏW1¦?´àÞ"s?_œj%Úý?J³U" ?Ù y8¯c?´¸å"~ªU?åö—2Oø*?©™¥‰
,?¡û̺d]?'R¿{´?ÑòR"6¶ ?¨mFٝ ?Ðæî)F}ñ?Á
½(@?€»¶‡šö?v(©°Õ­Á?çIšR|"?ÁGM"Ë´Ò?Ò¥'£ ß?Ãõ5¹AÌö?'ÿœ"¢ü¡?š™TÂ}})?æ:žPQk?Ä"˾?×[=hkN?´-jeÊ@H?¥¹qÊ°ƒ?"i'h?㸊Jœ0?´³Ÿ["Ü?ÚLk'HÞÛ?²œ?zš?±j.¶×?˜ÇV‹êéÊ?ଇù;É7?³¦+&¹%MIXED4FGL J0703.3-0050?Ä8'©Ì~@ø/0oÀ9ˆ²1@ìÀ;—'?2D÷@dn9ïdý@ƒ¯à,ûâ?¹nÓâ¯|?É'ÄÀ
÷@~…vÌå÷@
Àöäxe¿ÝO©@U°Œ¿ÝÖ
RÎÙí¿áú4CÔk'¿ä>¥¢fqÏ¿è1áÏh^¿ï÷:Êi²AGNbcuTXS 0700-007?ï<	â¤G?ˆ27¡>k?{ÖUèaú+?qÌù®ZX€?'ŠIM."?ƒ)'^ó9?ìƒv`?Áó?¶fÏ׋?r§ˆu}A?}&5œ¸" ?º¹ÔsEƒ(?µ€"æ1?îa3¶ˆ49?—jDÅÁe?Št5;Òè?ˆŸ!ÀZ}Ä?£OÀ‡š»?"[gFð†9?í*cR­t?ˆ'ß¾b³?†)pv<?bâ™*ôve?³é3ei-™?†Â.°Žõô?îTsëgË?žV¾gP¥?‰¢Ýq'
?€FÑ?¤P	îq×?šYSvÄ?æíGªþ4¾?ƍ]Z<ü$?‡¢o"^O?'ñÔ­¼G?Ñh]13~³?Æ%zå±?ì§íƒ6çÚ?¦Jñ«S€[?Ÿ‡)³
a‹?•P}¼3ñ?²ÞÉx<NP?¡è•øq¸¡?è Íì÷(…?¡|u‰~?©4ÇPï®?€H֩ፔ?ÉÇ¡²ËLx? 7,IJ‹©AGN4FGL J0704.7+4508¿å
+Ž¼=@5I˜ˆøÀ:ÇG'u¦À<hÇñ›¹/@ŠÒ¬_Å@@Ÿ}i[?ƲŸzQC?¸fœ«fK?îÑ;ÇVkG?ú"#xÕÿ¦?ÑØ	âx¿ã¼Å¸ÜU¿åX•Wëy`¿ê	âÂW}ë¿Ö"%>(¿ïð4í0EAGNbcuB3 0701+451?í—x‰|ì?Îfý4ÑC?NëòBþ?EP˜ßˆk?³b4Œ7?În¬ä'©œ?îÏ쩃hø?Ÿ'90ŸÆ_?'ã×ï­Z?Y¿\Ì\®?œÁxæÄO?›yX¶™gl?ï(î	Í"!?ƒŸµó?vw­nN?s†¼BÌ
v?•DSfæ[B?Wªaý?îlΒt·7?Ã÷…ÄåÍ?–Š€¬ú©?gúÎd?¤Ít9#<d?|QœôMµb?íÁC¡aÜ`?ÂbÚÕV½?cŸ#9?Zñ]"—–œ?±]ránÑa?ÂlÕÒk-‡?ìøF§sÜ?·¸ºut[?™\GƒÁ"ò?¯#8Ȭ(S?±æ¸å/b?°›)ì¬sã?î9Ó;Yzù?•eO;Ü·í?…õâ{Òâ¥?Qê¬O_?¦åS¨ûÉ?'}2%"-~?ë*¬Ä³h?›NëíƹÛ?˜âA»ý•Ä?ˆ‹£;ù?À;m¤yi?˜´tbé´XAGN4FGL J0704.8+4907¿ÏtˆŽÀˆØ@6BÅ;ËÀ9äz[ñÀ<8>gCÛø@¦¼õ¿4^@'8å#Û§?µ}€´Elq?Ö=C­Sá@
bô ά¡@.-ú'ѿ͍òÇ]L6¿âu۞÷§l¿ärB¬^¿éÍÃ\Ⴟ彵½¼Ž'¿å°eùRAGNbcu87GB 070112.8+491056?ïáýßÐp×?hd`9µ?UOhP©ï0?Zyt¡q?cZkê]y&?`Gٓ·?ïÛǝҨ?qw­?J¶]ÒOi¼?XÛaú?mŠÊ¢é¸
?jy3:D•u?ï¤Üà/?{!Á|h…?p6˜¾ó?wÎ /݀?}Z÷Àfó	?j=BÍ¥P?ïÎé8ÅÄ?Q©õ—$T?S"¼¥Ñò?3Ëâ|^Q?s¦'â#E\?O˜`‰Èþ"?ïÈ¢~£&¿?vÇm'¸?`·jÝ:ûv?_Þ v	I?sS8?þó?qÌP>?ï"ãÃÎ\?ŽÏѱZwè?at£×:Wø?më7­&¥l?Šiæ=÷?‹c\_–,l?ïPõèq?ˆáèÔ'?¬°Ñae?ÜE/û.?‹ìc•ü?|i¯|?ïiXµ½€m?u\"Q£à"?m§¬7ô?WL/t9?Ž?çzڋ?rŠŠÖ²Ò™AGN4FGL J0705.7-4848¿´õ1ÕAÀ1Øc8´|tÀ9Ö­ò2qÀ;úˆFŠþÌ@âs'?	*@Oï0l¯?¶®|Փ›?Å?Û¢¨‹û@
3Xòà\Í@½^Ä»?â—m¿öûu¿ÔB±Á¯¿ãx†YJôñ¿åûŸíp±¿çŽëUN.¿ïþu]AGNbcu3FGL J0706.1-4849PMN J0705-4847?î¬Nýéû1?˜ÇEd¾9š?'£ˆ€£›©?ŒÊe~òñ?—Ò—ÅŒš5?¿iŸÇT??îFJ^è°?¤éÐ?˜–,×ÃX¬?šoK^Åž?ž ‡hw_H?˜÷H¹fÅZ?í´,FÒCÒ?›ž¿cѸ?›…™3L›€?' Ø-L@*?¦únôéò.?"®a9ÇE%?ë;ô/gK¿?‡ë "×	}?¨yñÒx…?}ÇoQáh?º!Š$—Ë?"žÕÝ[?ë¿[cíª?±Þn"¬?±ìˆG'b«?¨0™²¾æ?°œ—XQ? ´ÖgÔpG?ë	9"÷ƒ?ºbͪ˜D…?´9¦®4?µ¶ÛîA«`?³|K*ìU?­m¶}ZS?ê0ÂvmÖ®?¯§Þmë?²»aT– º?£˜tcë'?»¾Š÷Œ¶T?¤Ý$ÿU´?äT»?uzš?›ì'ÛÎ?¾Ý×ÐЬD?˜He¤"€w?Ï>'ç€ò?š…›¤¼ÖAGN4FGL J0705.9+5309?î¡k➒Ÿ@7€ZpŽÞUÀ:Ø	ٝ•¨À<³Ð¡m£r@ÁÂr«Ä@'6~AN?ÁÂ˗´'?¥ùiãÉh"?åe'
@ž3ƒ:1ª?çÛ-¸Ÿï¿×å°¿åï
¿[J)¿àñ¦&oÖ¿áúw?|—«¿å¡àåÞlAGNbcuGB6 J0706+5309?õíÏ?¶@‰'[Žœ?if	\'­?˜…cBÒa?'z6-¦é?°dÁˆÿv ?ïÚÁåh$,?l¥Ào‹?DœcÖá‡?NWØ·0°Ÿ?p€ã$ˆ?gѦÚ)–¤?ï™äÒû¯?uÓ^CҜ«?_<ƒ;ý½Ì?a¬j"¾W?…Ÿ;Qpž?r·½ƒK¬?ïÆіhÀ;?Tb^Ó¢ºb?^}høUc?;­º¶›á?t÷ڑ¹Tæ?RuŠÃ€Yj?ïӜ¿`J?e"¨ÜG?T¢~pL‡?G,Î|[Ü?q	ÀÖZ¦?bM…ûÊ>½?ï'1lj}(?">ÈM›C/?VÂm|ùZ?`Mñ)j]õ?ˆÛL7(DÊ?'n
±4Ä?ïHèµPG?€.´4k?gž§6ñqÝ?Wx¿K[Pd?"ïuWðØ?}g÷,ì ?ï[t½Âè?q­ÔÆf?u$å·ZAæ?[1ZÖéBé?Ž]«Õ?oq_>+LAGN4FGL J0706.1+0246?´%Q|­!L@.beOæÀ:ýž5	ÍÀ<SôH;Øô@#½ÙI\ë=?ù"¡ò?ÄÚUv
Q?†o*bÝ£g?Â`|-Q?ùœÅˆŠÓƒ?ïMú^ÖO-¿ð?ïÿþó…õ?Ôr‡qxé ¿çää†&ö?ˁ%D@çAGNbcuNVSS J070610+024449?ä<쬳t.?ÐcŒ€Æ'Ü?RJÆ"Ü?R'Ý?×sÜjƒ?Ðblsh#ø?ån""ñ ?ÆBðé?QØ?‹¡g6<t?YžŠwÆ>?ÔEÏôZÁ~?ŵ<''A?隘{ì?±—@3Wão?jäÁSÀN?fj˜ê8Ï?ˆšÜ\.?±"¾túÆ?êvuè
?¦10¦öP?ƒ¡ï×Ó`ò?u¥Ë(Œu?ÄìҐ?¥ðÙ¨í?ãÚLQ½7?ÌnVÓT?[Ÿ­àó}??RŠñ«ýí?Ø/Ç®TçŽ?Ìq¬—´M?Ü dÛ2&?Êâ'T$;ì?Y( v´? pÊÝþ0D?árhòK¦5?ʙ¹úã
§?çü®‹ö?°¨àÏÝ$=?yÆ&§ ù£?s6^µ¼À³?Ñ^î	TßÎ?°–~ӌÝÞ?ãÍs_Ñ?¹_¬£a™x?—Ø6™ahå?˜?¶–'øh?Ö疎ï"ï?¹ª°Çwg.MIXED4FGL J0706.5+3744¿í#`Ê<œ
@2üð¸,,À9'dö#Þ,À;Ӝô—ìñ@ÍëZ×g?ü=³¥Ýu?«–3Þ~Ðë?°rõjû¡w@ƒZ'ó@=«2ž7ä?ïæ
öÔT¿Ùº"ÛÍпٔPdF{¿Ú&Y›|Ȩ¿Üž^$x…M¿ÞË(~»ÈAGNbll3FGL J0706.5+3744GB6 J0706+3744?îðÇöÆL?æACë\ó?o=;l†÷?`žÔ€óÿ?ÿ^3Uܚ?Œª7MSƒ?îI]¶-gÜ?³¶p-Ô=?'»ã§w?¡JåÊ«¨?¢ÝF­
"¾?¬ùsŽŒ)?ëéaôDh˜?¨Rœ<ޙ?'[¶<¬*?)½ìô°?¼¹1©4?¦£ƒÍ0s0?됶âÄu?˜@ÑYãñã?™
ySôŒ?vßûÒ@£?½9¨*;?–·Ÿ€
?î0HsÐöí?›!Õ©)?'6ï‡53¬?rd—;ÀÕY?¨m¼ãIÅ?™ZЋ<Av?ì=®fM×?»æ¢`èx$?£G¢ÕŠ?¯®MÒ8?´nǜ¬á"?´9áÃSý-?êòi"[UÖ?¬Ç*‰\â?•<1q'U?;ÖvÂö?ÁŽÓ"™N½?«5‹Èm?ç`vZOVÕ?® üÌ^?¦O?Q{R?ŠiÄĽ?ÌêVÂÑä?®"l3J~UAGN4FGL J0706.8+7742?»žŸ¹yC@;Gy¢ƒMÀ9kQÄòÀ<,=ÐE'Q@¯"}ûÙU?ýıû.·?­òŸïV?¾kdÒèoÁ@"ïï@Ÿ|󛘢¿ÀµÏš²sZ¿Õ‰æ]Â}é¿ÜÙhrLN¿ÜlÅP+¼¿äô,ø†Žû¿è"3ÿ
zAGNbll3FGL J0707.0+7741NVSS J070651+774137?ïö¯%/î?@¸÷žŠ‰?7T»@ók?1/
K#?I™qæC§?7k¥Mـ?ïÞ´P
?mÏíÒ®Ü?E'wô«?P´,FÇ?l›n*‰ý)?hùY™1?ïš­+¿?ˆ@Íɤ?z®™@a_?…aÓQÂ?x(0:¥?qÄ]ƒ»ü8?ïçQq.8?EJ½8J*?@aÉp%¸(?#ãÚe!O?dÉ<	ö—Ú?Bµz˜\?ïïÚÓö?S2çڜÙ?Eä¤J·ž?C‰µ˜úœ?Uí÷ùÑÀ?Isъ½•?ï v³÷¤ù?'‹~ߓ'×?W2ɒþ?d ÙS?"ðlªœM?€Yzâu³½?ïu+8›…‹?ŠÌmù¥n?'誢Ń?‡ÄŸå_¬?š<xtƒ?wû8cRn?ïÆRŽÜì?aMbh
Þ ?RJ£z?>6óGùŽ?xvT‰ÞÕR?^°ª¿ËYAGN4FGL J0706.9+6109¿ØâµÜ	E@9^=áâßÀ:>pɖ·gÀ<'UÓø@¬¿y4t@,ÅZèƒâ?µ¢7¢Ù‰I?ËPÿT'?Ö<á>iÈ@"IX¹"?ï &Ö@¿äȒ@	‹¿ç>-—è¿r¿áÒ6™A¿ç}§á¿åmü\ÝQAGNbll3FGL J0707.2+6101TXS 0702+612?ïãF]©Ë¸?]?@¯3?DÛ(/R?2ØÀs"¡‰?g'Øñ,E?Z¼È©ˆ?ïÓX)På?rÅj||Á?Mæ[ß´ˆ?VÚ]÷/‹"?r—õžg1?mpv³,<?嬨p$w¦?sgI±î?[MGål?c#ÎmŒ!˜?öN1¯Ü?p(ÓÙ¡?ïÅ ÓA'Š?Tùï­êäÜ?gEâF?F`ºPœf?q­ˆ¬fñÁ?Mèx;IÌP?ﶩ#8?v˜º;Ç¡«?V$>­ ›Æ?D¿ :æ—?"fµSLñ?uz0·É«"?Ø^6¨?‡ƒ3
JZ?[h¾åW'?gà©h» –?Šë}ü$ì?"Û"TöÂä?ï\ÄC¼Bf?'°\3£c?f>¾H¦ë?g'ˆùy®?'ŸŸÂþlØ?€½ÁÓߺŠ?ïN)Þm*?tíÆí¼½Õ?'™œÀç:?fcHÑ·a?‰Û뗠íŒ?mz÷5_ÂAGN4FGL J0708.9+4839?ÛçUnòQ@6Ɉ;£D=À;IÐ&ô`À<Á½"¨™@!¾¢ªdm?ù~{?ÑΝœ…?Ãfmé~3?õslg@8Ë0šÂ¿ÛšÚŒ¿ïÏäM?êÏlº=~¿ÙèêÅ[>j¿ÒÝWžøS8¿ÞP?þªJAGNrdgNGC 2329?ï¯,è/B¨?ƒËâdŒ81?O3τ3Xœ?J1§H£9þ?'A‰PÆå?'½c¬"y=?ï¢5)†P?"ªk¶ÍÖ?Zvˆt©à?cŒä"ðY`?"#èýVð¹?·BœÃW?ïCw¾Ódì?ß]
Æ=ò?Yð~T²'?HÎü,^©?•ò@ 6Ê?*Ù=5¥?ïM†_o?y7ˆ$± ?S	´IMn?Bê§K!s?œNÛsT?xë…Ãý‡?ï5'Ï˯Á?Æ²¥ð?bdKJSzÄ?X}>ð¯Ã»?—<—À8…?ºx-Û|à?ïŠ9?Ÿ"`+̨?hÒvŠøW?v©‹VAI†?šÞôjì?U<¦9š?în$uk^?'wUË.T6?a'(d­fœ?TúH-sß?¨Džî×´?'CIÕåé?íc¦´h?–1¤Þ^T%?^'µ
VíZ?V}·½#h?³ŒD¥ÚM?–·@1AGN4FGL J0709.0+4304¿±Äž¤3Ð@5-j½ãû½À;—ߨq£±À<žÌN!Ì@ N33²à@tÛ>—?̳Ä=19¿…˜ô`Ãô?·B›îœo@´h"ÿ‰¿Ø>\œŽ­¿î{ ŠN£¿°©»¿xS¿èä§՟Ú?¦RCí²1¿ïÿ¡ ÏAGNbcuGB6 J0708+4306?ï'í¢<E?‡ø'—T—r?S÷)…?Þ?P°Ãms&?ŒÅµbj0à?†ö#T$?ïXmÓÕ¼?½7@yç?d¢Š²2±?o'C¡ÏÏà?']õiÿ.?œg#Õ¼?–~ ?"cõ‡{ëÑ?g̔ùÔ?j°L0«©?¤ÔÙÒÊ?"OŽ‡?ï¤ù\š,?iEPÕIØ?-*v9FNÞ? +}ìâ&Ï?†ƒ×ÐóQ?i<
ƒ³?î"
uh¦¡?¢°F°ó»??hã¤h¡Gm?i|a£Qµ?¥A`ñºö?¢3a9'?îÉV–mGà?«/rØfhR?p¢{°‹Å?'7Èó"+Ú?¡VG<-‰?©î´Èß?íñVä‹?¢²PĚw†?saìæˆ?t–¶^¬J?¶bY(Ÿ¸@?¢†tSž?î¤{5'˜?Ž˜ËºêQa?F˜ÞÓäÍE?C«&"S=v?¥]é/Ó'?Ž‹¥¹ÒÀAGN4FGL J0709.1+2241?ëÒê'äv@+ªºà;>šÀ9Hôá¾ÌYÀ<*2	@Êi©;ù?ÿí…tH§9?¯ΠÑ5+?±k
?-½S@t–'äZ@D!ÂóZ¿äÒ-^ÝÛé¿Üeށ*7¿Ýk¶Eê¿áK—þŽæ¸¿å_(뱔¿ÙQQAGNbll3FGL J0708.9+2239GB6 J0708+2241?ïôÊ­ÁLo?Eé­9üw?%¶ÞS½Ç?téºïEê?S³È­x´?D†,Ë1k?ïâø¯m…-?pHÁ¼*Ä¡?AFµ«{?O12Mrû?hµÌü*±ý?k‰@»hk?輻,Hw,?|çgS³r¿?d°"¢p?tŒN6¤?€²Þc3?rÕY#·ß
?ïåö™:?HFÒ¢¦¿ç?@=(ï¡|ú?$Žu"W€??eú4…^÷L?EJ"ÎÓ§?ïîPBb¦?Wºàz#?0"¾²ŽU?!®†·Éè?_:‹¦@¸Ù?UÆgqÂÿ³?ï¦M9CÃy?‰Ksü?Q‡JmQ´?adÖÙì÷	?";Èdԇ)?‡;eömÉÌ?ïu]Qê®_?w¦ÂÉ?kP‡$¥?tn¸Yu?‹Ô‰¹å"ù?{'üžÚ÷·?ïäBržâ?cõƒ1È®ì?R¦ü_3??LXðÀ•Õ?yª}í·@?ašH-'AGN4FGL J0709.2-1527¿é˜§7«¬°À	0$öYŽÀ:–æ`ò‰À;øªLb@!€¼&'?ûÖNUÎh®?Á˜kܜùu?½j§=Ç
ì?þì¡c'v@Y1(¥¿ïÿÝ/ñ_S?ïÿþBe«+¿ÃGahz½¶¿ÇeöÔÞ¿åK
P»Ú¿¬:XŸ¯AGNbcuPKS 0706-15?ì6?ƒB~@'ƒ?JUý'f?A¿¥Öev?‹Sð+Çe!?'Ä@ðZ¥?ë-
"í¾?Áža#X¥?]ã¡ù°Í?pï½ø©‹ˆ?Ã14wÎ?ÁbstŽ>¿?íü*0]Ég?š…鲍f?xq"Ù¬â?}µ¸» 8?­/*_í?˜ƒ7Õúá?íÈQD›?†h˜y	á?zËé ?Ã?["Mz‰—?°Äì>D?…§—`º?ï
—õ¡ú‰?""~Œå[?cù.H'°?`õ0ï;?›Íیûrõ?'·öÄ‹A?äLâös©?É}äv%?m¬ÛFî?€©šõ
—×?×Á2ádð?ÈÓí䅷K?륓ž¦Ò?¨&ß6®2?†ž­Ìùº¹?…Ó÷À>¿›?¿ÿ¿EК?¦¡ƒ­§¡?êÚÙh<?œhˆ‰å?	~ÿ›sg?v·OgêE"?ÂÇïÄÀÜ?›_*Ì¡µAGN4FGL J0709.3+0540¿ê'…4@@W_bf'À:7a=1¹¶À<1REG1î@KÓòZûÏ?ÿ»°åæyF?Ä@jS…ä?¸HQÓ\?õ:ðFN˜ê@'P(as
¿ïþ`ù?Ÿ?ïîLC¥q>¿çØ#­"2)¿Ð®#¿LÜ¿ãˆ$A'è|¿à8L­W¼AGNbcuNVSS J070916+053901?ïRBiðµ?†úé×?NTÍIQJ–??Šçð#3?"Å¥ÁC?†'YÒ}h?îß˜W^?©ýZ8y¦Ý?V	AÀ:Rl?ežÎ…ü?¦A¼nø?©D²k'\?î¾K
6t?ñáKj
?o'€'µÊ?hkùÝUú?¢"=S³áb?Œ
Ú}?ïlŧ$ع?iÈpòY?g9•—;Nj?EŸ•ÿ?0Á,ÊR?g©·mÅÎQ?î~ùf;Q?ž©ŸW:ýÂ?[Ì""›/?Mªu£´êG?§2ˆ
?žPi‰Ó?ëþã‰8Á?¿(€nz\?n»£Jðƒ©?€»C"¢¼‡?¿œ@+Ù?¾Wµ´yÓ?ì°¸ÊêÒû?¡•F3ýÖ?T?JØ;L?x…z1ƒ2Š?¸O±¿N`À? ´¸óµf?T
u?'é'rÞ]?yóvëÕâ±?aŒšƒ??¢‰KåþïV?k¶Î…ùòAGN4FGL J0709.7-0255¿ä¿ÞíCÉ@åc>"¹†À8†à66òÀ;q¡3ÁÎl@of×¥mã@¾::ŽqG?¥­ {\?±¹_°ƒ…@	•õB6Ü5@T84ÏÀr¿µVz\'}¿ß| $"I+¿åŽ¨orŒ¿âh‰¡~ëC¿çä¢ Ñ±¹¿ãHhÌAGNfsrq3FGL J0709.7-0256PMN J0709-0255?ï¯Å<W³?rC%ù¹°?=Î\ZW\?0"«5µïw?ƒ >H?q¯h^gÝ?ïrMÙbîs?–@¦ŽI¯L?F{AŠåŒt?Wy€14Ü?'jÀ£?•Éöº¤.³?ïbRÉ.:Y?'é5PS[p?jæmíÙ?pJ)Ÿ®­?uJ¿;?€s¾¹®à?ï˘Úi²?Xw£Iv?C žbãK0?%†K(«'ª?wÏê´Jg0?Vß݈¢I˜?ï${gk?‰Èªø=s;?H^ùö[…L?;¦¼u)?š­›:J×ÿ?‰jhÿrçS?î
l_Ø5i?³];ÅSá?`!EÊ5€?nä
¯¸¹H?®'%¨™g?³HÁŠ°e?îãjÀ_£v?"U&§?wªýµœd?}~D"î?§èŽ_®Û?'˜!§ùx?ï'>Kó§
?ukæ|ÒÂ?X±'ëî?E{G0Ò¼6?ŒZLú?tL°S5¯TAGN4FGL J0710.4+5908?îI±Û‰.@9lÀz®òÇÀ9ºÑ4:š0À<6ÙCӔg@!‰Á	u?ùâTÊ\°?°å%´¢"?¯9±$P@º?Ú
¢ñ@
'Å—j¿êŠˆ_	¥Æ¿´#7èy¦Š¿Ô$«°óRs¿Ðpeƒ<Šö¿Ü¡ººÑw¬¿Í_9÷GŸ§AGNbll3FGL J0710.3+59081H 0658+595?ïù'ÿ½ÿ™?7Ø/Քº°?0!"_¯?
Zœ"£´?F-üûŽ?5ó£9Ùþ?ïà_ö­j?mñ}TPˆ?B*)"%cC?Lalðž"?k~«¥_s?h¦\]<ˆÕ?ï¬èÍ´î?v©µ¾ŽÖ¨?SBëèñ‡?WèUHlºm?']oZˆG?uÇx 2ä|?ïŽùs…?cŠ
^ßÅ?^
‡•´?>ý‹br†?ˆò!Ç°@?bp`G`å:?ïõÕw@SW?D0':¸\¸?+ØO´È)¥?!Y@þjÜ?PÚìˆ&ô?A«'‡¯öÎ?×å¸4?"–DïV;?U(v ڟU?bӜpHÈ?"t;SLµ?'>µ‹Û?ïvˆFyÐÀ?ƒÊ±¼—?UgŽ3{ÙÈ?H'-Êˎ?°üŸ"Ò²?ƒ˜7ÀEàÌ?îï~¡Ö–?€‰±ïL»²?p•·Làë×?Y¦WÝ'‰?ê¾{îM?w0'‰ÐAGN4FGL J0710.8-3851?ÕÐ:k.ÅÀ*E{cM­2À9œFp&ىÀ;æ~AN~é@õ£	ÚÊ@ž¥·µ?·ûRò[²?ÆRüýA@"ô%×*@²§|0R-¿á•ú=H_ë¿àƛÞÚ¿çöó<¿ê;3¢™Èi¿çʃÁd¿Êëï½<¶ëAGNfsrqAT20G J071043-385037?ïú0ùç?7–Hoݱ?1aÊú@è?%ÊŌ†6?==,á½?1^Ïèæ×?ïå8¡Ôs?qnÌ>š?5ciN?C>fíü?h(uµþÅé?pM'ZÌÒ?ï€÷²å¬(?š…ÉÎU¼?lBk_t"·?nñJÐr?ˆ±x]‰Èì?~ÌDcŸž)?ïÀý¥v‹f?\²̾ŒÔ?U*N^çÿÊ?9œU«¨M?z6™¯Ö?[Ý,ñàÃ?ïöBŒ
+?E…ËH\Y"??bÁBGg?7+QåÂ?GDo¿áúµ?<ÝBT–z-?ï·#|JÃ?ˆ¢'x8"?S·?\åEÙ?mVv`,Ü?€rtì¹?…!s>ÒS?ï>æDÂþ?à×c@Ã?|]f›<k?}(œ‹L^?–ɈÝz=?‡æ7¢›°?ïيÜx£?ƒÎ§Ä²Óy?v
"¼0~?bÄð=tê‹?˜'-}wá?'Ü"ÔÔ@ÔAGN4FGL J0710.9+4733?ï½ÿ$Á^@6Ìt§qÉqÀ9ýçÆ²À<Owï$æi@¸Ä(äOË@ë꺝 ?»ËA1xö?Ãv.^b@*6âëC@y	³ˆB?ï!#}´¿æY*Fy¿è¿ÔáïÛ¿çq·20Ô´¿ð?ïÿÙi"A'AGNbll3FGL J0710.5+4732S4 0707+47?ï÷Ľ)l?Tص«"?CEI²à
?OUpÀ"F?;OXL,1l?<òºª>-?ïÅWšñˆn?zŸþ€?YõL|>Þ?d€M'"½g?vÖßpv‰A?rB<¾áÍq?ï•k«¹p"?~½¯²{µ?rf.Û§/€?uÑ™ã¸Ä?qý«·]`?t•ë<a?ïÝð¡ÿ'?Rt.†šs?\ÍR¤TÃ?D"BK`)?c©?0ñÕ:?H¸ˆ¡ÉL?ïòÔHl*v?\ýZ	¾÷?Sšsô~?W²§#DN¡?=OSíÔõ?A}…ÇÓA?ïY!"ðږ?FkXÅgH?qºû·Æ~H?Šå¦.õ®:?m•&ê¼?'UÝ;ä?ïAבÝô¤?‡òŽL?€©7Æ:?€+'ú˜¥d?†è'Õ?¦ø«Ž–?ï}¢}Ìg*?v˜^u_?}ßBÖ?hnx=?']‹]®?l7MßòµAGN4FGL J0712.4+5724¿äR±íg:æ@9ZakTãÀ;s\,PÀãÀ<µîj¬FE@"(évј?ü-­$ß³?ÎRœ-Q?¯ÅHŸ5Û?ã?Ðà@ÿ'¸ÿ»b¿ç£æߝ‰é¿áÅâÝÛ<ý¿ïš@2 ?æÿOÁ^Y¨¿Õºt»=Ù)¿ÝÁ'œzIAGNbllRX J0712.3+5719?ï¯`b7Ïò?ˆ5¿eÂ7Ú?:él6Ÿö?1ê³ov{e?ƒPœe?ˆ­!`Å?ïصíÑîä?uÕ,òÆ>e?DœÕAU?_±É†'ü?qnx<×i?q"׸ß?î¬Ñ'œ°ƒ?–ýÆӌÐ?Yr«^0?bÕÛ,¶‹?¤fì?¦*™?–Þçå(¤"?ï¾'Œ>¶?l¸Dkžv?9¿4/aLÔ?2¡‹r
à?PFÌ
¦Y?l{$º"¾Ú?ïœÁ»»qJ?"3:ýW?Dö.4±Þ»?@rY+}ö?‡€.=ÉòÏ?ƒÀ™Ñ¸oú?ï4k ¼?Ãw
8î'?Q/Ӊ׾?b ì—yv?‰Ì꫏MV?ŒBÃ
?îGÀÕÍ?™¹ž²õ?eâþñ™×?qèVë'?ª%Î厌6?™^Š¶ïÈ?ïЌÓk*?]=¼±É'?`r½29'?a}€°#U?7–Á¹Mˆ?U†6"ÏAGN4FGL J0712.5+3311¿ãéą38Å@2Žª:э&À;€y1DFÀ<¤ªIë@ #÷êï]?ÚI…ÚõÚb?ôj\_|gZ?îûÀÖ…&?ó¿hæsg@˜'°H1ȿ畟¿MˆI¿é¸;Ÿé¿îÍD¡š™õ?éÚFsBî¿æPÊï¿ïú'`åóåAGNbcuNVSS J071224+330953?îÃ3õ©†?¤ƒóŸ\m?m]9%?q†?‹Hñõöó¯?¡öí)z…?¢gÇ©;<?ï*ǘŸ8?™ÂÃÀ{ß?aÿÄ4¼?wEÁ•‹ñ?"5]
ñ@b?—yE0ù¬†?íH;õhf5?¤i(û†OŽ?}æ[^‹?€Ùw¯~Ó.?³íñî®ï£?£Vq̂t?îóQÞïå?"N°v±¶g?4Ifv²×)?G©SM®Çµ? ¢OB)è~?"j±ó¯D?£ÕÃÓ?¢·'ÜÀj&?}Ú´6hö?|õ׶xu?¢hka>?¡d@èŪ-?îðÍm0¯ö?©qÆ>XÏQ?u=,ö¡/?È\7©Þ?œ—$(פ?¥Û`†¥˜?ì´0s1ÈF?¦¶aJyŸ?~`½"ZK?€«Ì¸NS?¸xp"¶·ª?¦vs¤½d?î|Âv<r?¥9´U? ?h#-µ?;cò£Û?¨#ˆtœùº?¥ËT™ã«AGN4FGL J0712.7+5033¿ïZúXÁ@7Ý÷¯îpÀ9ʉ%®À<9M÷×ü@Oô**¡@wڎVo?¤)#~¤?š<&]#?ón_ċµ«@®B"ùF¨?ïÿH˒:¿Þ±	!ç±U¿ä)S€°"ˆ¿ã¥Ž/L¿ã{A–£E¿Øºùe²€AGNbll3FGL J0712.6+5033GB6 J0712+5033?ïíhmú?Q†b¨ìEØ?&¥Ëoºy7?ª3¨OÊ?a-¢á'?Pì]=æ?ïãqJΎ?m*™oöÞ?<È]^fÁ?HÜW·Å?hà•ÒÅÆ?hÍùß0ÒÞ?ï…wÎ~±?"|´®k¨?\Šƒ²À"?`qªÑ.c?‹îÆ ?"U{dÖÀ€?ïïuy‡^?@©'2-ê#?AA+z.{?&—­3­X?Xtwoþãœ?<
±'V³?ïÛr÷L¿?f({4®ÒI?1JhË;
?%«ø‰?q1Ýãÿ?eyÍßæìÉ?ï§ý"¸*Ì?†Š'ßã—ú?QŽ9Ȳc¥?a‡&÷?ƒÎÓ¢Õޓ?"*
{°ÓÝ?ïf—c´Z?'Ø€|jžT?eyñò2÷?a7íԚ¦©?›îՓÎ\?'ññÅ5Ç?ïÔ<;UÒ¬?`òÇ3	Ÿ?X "U#&W?Eã É¬H
?o³zo¡Q?[;)ç"+AGN4FGL J0713.0+5738¿Üd…ˆë@9wt¼j~úÀ:ª‹#À<[AE÷@sáo@Î@Ãa	/T?µ±¿?Æi†?µóãqT?þ! v˜Ò@úÿý{ÁA?íjAQÙçh¿â•?í«À¿åÒ<öˆˆ¿ã£š8ûÊ¿éf\፿ïȶ`x'AGNbcuGB6 J0713+5738?ïí†p…»?NXz
?;¤—ø¥ZÒ?)…bˆ¥'ü?^	ú%Âu?Kk†ß7¸ã?ïè*xúg»?iM¸oE¦´?=5^A0Ñ?LxKÔ׍ß?d.亗O™?d}д·?ïÂÛ®€Ë0?cpºêÚyh?XÁ(ê
?[*löÝqR?x‹øƒVý?YöÁÅ|]?ïð£§Ëœ²?>W.ښÖ?; hÄòk?!d¶š>3?Wð–îõ?:ÄG|$?ïÛZû_mŠ?aTÍdßÂ
?Kꊈ­,?:+9]ʦÇ?mªb?ie2?_ÔÄ´ð£?ﵗþ}¸¬?€ÿÔ®dú"?PvL±ã(5?`DR {y?€‹6½Fëù?~@†!Q'O?ï&Ê«E¥?wçTÖ¥¢i?cæº3k?Xaø—"ÀM?‡<žÁ̓—?tŠ)¢Nd?ïÒ½-·7(?]ßON
d?Tœ™ó…?@šß9±Iû?qzBºÝZ'?YÇ
®UAGN4FGL J0713.5+2537¿ïÉÄgu@/Ù¾ôœõoÀ:¹×†d2¯À<ƒÅg}¾@¦¾p=«?ýǝÓ[\?Ðú±AV¥?Ò—ÀÑkî@Ÿ¿ž ß?üë&¢E?ïÿHµ{wp¿¹ò4æ;´¿å±æÍ)¿Õð9Õó<¿í¡Š~ɉ¡¿ïçôpÄÜAGNbcuNVSS J071336+254016?í|º›ûQM?¦$^9^Tü?~Y °_:ñ?uþ7UL?²4™¢i?¥n
ž ?ì{^V]Àâ?·£-6Üðb?£Ø7#ì?¢u!€ˆoˆ?²9D@A|?²·²"Ýå?íLêgE5?æ0˜pœ?˜¼äóS'?'VY¶§1ã?®Òçlu#?™)ƒÖ ð?ë¢Ü.d~?"ÈxÃá?©HgãWí?‹E¾¼møå?¶DßC	#œ?‹ך"pÖ?êêøÔEE?¶™šuî‹è?‹jÀ(©¶U?€èÌãÃe?¡Úu
?¶(=áI÷ê?èÁö¹œ?ùùzC¬Â?³ž¿åôì?²lM:—í?Ã(Å*/î?¿©ºè¸}?ë"&Ú¤·?¥âsÛ¢†0?¢0".>†í?"ßì¿
u?ºN¸SËÑ?¢G L"Ì?çPR-ìš?¦€C\œ?´zgãߥý?žšËjC?ȂfÄ|"œ?¡QÊô–¦†AGN4FGL J0713.8+1935¿î¹ü>ïê@+'ãÑÌÀ8Ü#™b<5À;ØߑËnÿ@_""	"@-ÍbôÁÞ?ª";}üÒp?»	7¡¬ãx@™ûçl‹D@µˆMÁÔÌ?'%f ‡¨¿áˆÿ΁ٿå4ƒ•KV@¿åãÃb(¿ìçù¸¢ž¿ïúÈRꈟAGNfsrq3FGL J0713.9+1933MG2 J071354+1934?ï«®ƒzb6?tý`îvMŒ?`MàrðÝ(?RØ/"Šº?ç1O?røiã
uó?ïÞÆ9S;?tE ¾i?AÂLŠÈ`ê?Rló!‹C?lÉhƒgú?r`ê #Ç¿?ïi÷j·.?‰1 *å([?zAø'â<?€Øðë9ÈA?ˆa l·,_?qÿ»ÓPƒ?ïøAÇ9~Á?4ŽU—? Ö¼³/á?Â#‡ÍÌ?JÃ3qE—?2+
	¹%G?ï^a.ïÔ?‰Kt"ô»¡?gízoÇ^?`¡a'²'†?'6*Õà·?‡M»Èä"
?ï©@WÖM!?‹E6ª†ÝÇ?Q‹ã˱a¿?b¸¯'^ü¸?ƒ~m"1Ÿ?Š3%‡"Þ?ï*Cí·ö?'3ÉŠ;<?ƒX!²æê?ƒc—îî?–.¦§6IÅ?#5/?ïìáDŒ?R',¶âî?4ìÚ¸+Ðí?)F/㮐?` ·¸8?P{^,AGN4FGL J0714.4+1110¿Ò"@`º¢J@$H÷‡‹zÀ:Èû>ÐhÀ<rŸC@Ùî»4@¤XÍ?ÐÙ=^m"?ÃØáty¥?ö¡]b±¦@|Wt0('?ïýƒÿ("Ÿ¿ÝûÙ)Òa¿ádže0[¿×î,-…tI¿åŽœ`w	¿ïÿý¡UûŠAGNbcuNVSS J071416+110830?î}¢(oœ?£ /·?e¥áë0ÔÎ?cL« u‹?¦Ç¿¡ßò?¢ð2²£¹€?î@}sž2?§g;ˆÎ7‰?e8Eà—¬p?kø—ù××ù?­èsÈ(í?¦žDN8*?î=ø~ßâ‡?™–/âÚt?u<	B?v@WNk?©lД«¾Í?˜‡u0ç?ïX ¯QU¢?fØæG&?gà^‹`?CLX#÷Þñ?'ûî¬Z?e9ºñ‹þ?íμ'&š?«¼vëÔ*ã?nˆCæÃÏ?j=ˆ">1?°•Ý¬«à'?ªôó¬fy&?êóÍ-?ÀX+žG?zÕÊK

ú?ˆ#ÈÞµëO?Ã[Jx
¶?¿~ŸÃ)_ö?ì;cÿêí…?§R2Ò?…HTÃÖÍå?ƒú|¸Ù??»{ÕlI"?¥¹á;-xj?îJæè¤;+?''~šs4?wd'ò¥•L?`‰¬‰+(?¨dÿ…z+?'YÄYó#ÁAGN4FGL J0715.3-6828¿ïÿxô(uÀ6øƒ‡ß\òÀ;i•ÅσÀ<xÉ7Ã@šh®ëƒ@môݍq?Ä<Dÿ¹^0¿œsY>	Ðä?Ø#"Øå@.`÷炱?蝷€µG?ÊOø{QZ¿é¥b$¸F-¿áÖ3ž$E¿âešŽŒ^¿Ð~Dß-!¡AGNbcuPMN J0715-6829?Qî›e?鞧èí5?P8Ûï¢#?DsÒ(Ý4=?ˆÐý´‹?~–§y'žq?ï´=¥/­u?z9ú§x ?S¦vc?µ?XIމxeH?€{Çç¬ÂV?vª—É*ðà?fr•?–VbCÊG?pXÜÛ¥½?wL~Y\s?£~(8	?•gË跔?ïwWŽñÓ?jâ1™›>*?\0›LxÞÌ?A‰<C\wq?Ž¤(¯DÓN?j!YjuÜ?ïI© —œŒ?óAŸ•X®?cE×}
rˆ?[ľñwèù?"b!'f4?hëÑË?ï,{oHH?•æîìDQã?bÔKIlí?o9݁-ò—?˜-aÇw?"|…3Fƒ'?íçÓ&5ÒR?œÛ¥[-s?u<¾Xµ½?vðfÓFU#?®Û5Î̉ä?›Î`ÕëŸð?î5Þ^D®Ü?‰H'Î¥é)?v¸ö"=Ö<?dB» þ?©ÊûJë^ÿ?ˆ®øAñAGN4FGL J0715.6-4528?äþi°{fÀ.
_V§¬'À:.ÄBº³À<S"}¨¢K@ïE…pB@=Uæ¼b?¶šõº¿rdœBÞz^?¸"~!™ï@wNö³%1?ïõÄr‹7׿äãü":µ¿ä‡.]
¿åÓPÊï¿ëüœ#·•?Ûáad°AGNbll3FGL J0716.0-4525SUMSS J071544-453031?îùK=ôŠß?"É´	IG?h0"a®µ?_G¦´Á‡"?Ð"«¾Í??"ávq˜Á?ï͏[ìԙ?vwº&¥æ?I¢¢U¬kø?PZD["ú?vý µ-Ó?t1͉QÍ?îçèÊ.aè?'¥F4½'õ?ƒ>(pÀ¿?…o#DçJ?™cÒ}ßÖt?‹f•v¤k?廊?hz?a—<10'?cîü'Ø"?D¯Ëwó€?Úmèƒc?]ìåE®?ퟓI¯‡©?¬íÒôâž#?"ß%±iÁ?s1zbÒ÷?±7¿AÆ_?«ñüL»FG?ïrþֈã?•4ɂ·Í.?Ytš*"õf?eDžI:‰N?õ†¥,<?"KŸ—ˆ½ì?í¼Ó¢ÿÊ?†ŸšNE>?'ì𢢩N?Œ/£-W?«HºwîJ·?˜?k¿«*?îùZí6yº?D|€à?|:/é.2?eCµu~m?™ÆWãÊH?z*®$L,ØAGN4FGL J0717.7-5519¿èÁl¶%…9À2zîÇÉWÍÀ:õÈ	ïmÀ<ŸµV¬µ@ úÿ£8Ô³?÷´º6È*?ÒÉu)wȎ?ÞÁS<=@âݽµØ•@·a·?Ôúß?ï]'îY¿äÎ˪Þ?µn˜K»À¿álN']‹¿êÜUÁR›-AGNbcu1RXS J071745.4-552024?ï¾bŸ: ?'œ}*¡^ø?TX7NøÂé?Lc¥f¦Ër?{¸¢ƒƒØ?'ˆ"]>R?ïà¾
?¤v«'ʵ?{K§¯ûg?†ˆ£È´žµ?•›Yq½/ì? pÃÀíB$?îí§)hóÎ?'L'‹Ð†ª?}‹
`¢ïd?~:y\º?šèWƒ#ÕU?ªT¼ž@?ì"ÑÎ
ÜÊ?–pÕ/eÖñ?œÓÁקüq?ˆJWðŠtÁ?´¤L"?'øÐEY#Ó?ËÏÄ?y°
@%?kbڞ§4Š?dç@:µ?€?Öj<':?sâCôLö¯?íX_L84F?·PLØý†?›
KÕÜå?¤kü³‡eì?¬«""Ùÿ+?²ÑÔLár?îãØÆÄå?Ÿòi™•?‡¹ÓDýÍ?…¨ª•?©"MŸ!F?œTñn"?èU"!?ô??¬3\Ò'¥l?ªmm20Êe?Ÿ#¨\È0p?È"/é¨?©½3ÚP'ŸAGN4FGL J0718.0+4536¿éêOy1f¢@7tàP7PÀ9ÃJZ—%KÀ<G'ñ·gá@Ls 3&@û¥»ç?²°Õ_îR.?Ì-˜ªwŽ@o1'Y4@*€='(?ãRâ/àm¿Ò]³ß@¿ç4~!nÑ¿ç ÐàWÄ¿í ìt2¿ïúöv'"AGNfsrqS4 0714+45?îìŽÿ6×X?«¶.M5áæ?–Méý;'ê?Y´½'m?ˆ@lE'J4?ªã­¯îX?ïÁ@"-€?€l£Yž?_iHä5wC?oât=c¨?w…©þ»º/?uå]7Iµ"?í£j‹9. ?¡uy´äÞ?¥L½•CÀì?š¼™+"4X? |™µq‡?•ÛUmô
ÿ?ï ­¹P?Y	QŽ^n?gfNõxÀñ?Jd=…¢™?s< \Œ?QèËû}y§?îWS¿ÖÖL?Ÿfïў=¤?¡Ìé"ç?–ªF².?'Ùî2«?ŒD×Á	¯ˆ?ïDSËw?©7gç™!'?rJ±J)‹?$å÷òé?'Ò3ù]¢¾?§dßߖ?ìU(èp[!?§€ço[¼?­+>ðq:×?ŸýXå(Ì?­'2…w#? aˆð¤ÏJ?ïMÁ%Ç\?z'É·ˆ³¾?59@; ?jZèº,L?‹Z}MS]?r²ðêx®6AGN4FGL J0718.6-4319¿ìÓÁZu8ßÀ+OíA·ZuÀ8œT§!A™À;'³ k°@ß¥ídó?ü¨J¡äÁ¶?¤Ÿ¨@?O?¸‡žß–ä@€€B_@´ jÓ?Õá¼'-@¿Õòâu«}È¿Ý÷:Ÿ
Kî¿ÕÚJ¤>
W¿âŽÌ¡ƒÈÍ¿çÈ}GS{¨AGNbll3FGL J0718.7-4319PMN J0718-4319?í­²¢\·?£óOŽÍ?‡ª3H@†d?ƒÎˆxYäë?¯:Q2î+ý? îöÂdu?îRKdµê¼?®æ üfýÂ?•`yvëB#?žÛ'Ä_¬=? +ù+³4?¤"T·æ?ëÂ
ØjÝ?«—eíÝ£?¢.sq@þÜ?™šNªšäA?¸ØuoRO,?¦½£|*û?éuöêW¢(? ¥³š?£ã
^¥=A?€†`n5*ð?Å/a¾A?  W­°Y?éюœ ë?µ‹ðb`ïÅ?š" )p[?"C3œ¿³?ÅuƒM/'F?³®t'iï`?êߎүÿ{?ÃAò7YLf?¶Tî€mý?ÀT,¬J:%?²¯u|Û}'?±{AT^&&?èrÓ®W/¬?³
'ž"ƒ?¦tž°½t?šÚîY¡?ȗªŸ.µ?±ú³à£¶?ä4ÿÓ¬²H?®2`åÈò"?±—h,ˆJò?•áÇ"iõ?Ó0&Lߛu?°fn<"HAGN4FGL J0719.1-7055?ìèLÒcÀ7R™ú©vÀ;Ø©yámÀ<£Vh•ì@ '—)§Ä?ýá¥Ãsˆ?Ìý™ô2ld?ÊáYv¾Î1?ý§Ww¶@`õÏûUv¿Æ¯h¸P?ïÛ }-¨? 2=ûõ?™¿Úoø æ¿ç;Mlš]¿Îyz?a>ßAGNbcu1RXS J071910.3-705411?ïáñ?P€?[ÌGNò¤?BÚ00PßÜ?2©0¸Â:ƒ?iX4Ã*àr?Y€â±ÅP?ï§C@˜?~øÜ'c"?\'ëÕûÆ?bP¹_>uM?'¬/Ð~?y{ÔéÒH?ï{žÁ?y=.áù/…?eEås''?eþi¸bú?‹ìžóLr²?v½F¡Áݎ?îže§iÀ?}úù?†Ñ"$á?fÔrÉyBÐ? eDŠ@Å?xĤh4[Ï?ïÀqñE8U?o^‡;rmÃ?YþL8@î?Lí·Â±"?yGtPqx?l
øO?îøãºúè?™jJ{Ã'¯?v2bž?‹V
süp?›j6ðüÐ?"¨H*ˆŒ#?ï3'i–¾ë?'h9fl"?lBuú@?iSÈ3rä?–"&ÕQ¸?™Bچ!?ìäØtÿ9?"Ùw«U4?"¿ëÙ2¦?¡±]?³©A–†f?'­0€,AGN4FGL J0719.3+3307¿îzl¡O+È@3Ü£}™‰À8‡Á*[À;§Ü®ÂË@1<¢ô@¨l›3͍?œRiH1á¾?ºctïk2S@ 4çhY†@cÇ8ä")?psecÜô¿Ýû÷|ù¥É¿â­½½æ*¿ä0Ž]{[@¿çTèÅP׉¿ë`B5ÃAGNfsrq3FGL J0719.3+3307B2 0716+33?ïØQâîÄ?iKÎq|îã?Qhøò܊<?I¾'N™Â ?nù "Yn©?e>')Múß?ﱃ0Ý©¥?'Às´=ðã?XÞt|@"É?d7}Ù>?€ƒe:ta?S"ә?ï›^ÌzR¾?ˆÓ9ªDz?uجG§Ï‰?'KÓ¶•"?|wí"ìƒ?~¼Ÿ?T?ïã""DZ?Sâà–…A?G˜;³³Ì?9^MÜۜ™?f÷æI|â?Oxyq,©?ï¿Þòêá?v烳Öí?Tfº›=ƒ?PQ;©>ã?zö×ÝT?ubãeÄ[?ï8Øó¢,?Lo°á?nç;.ùî?zEa?•üaš7?›ß¢ám£?ïhµP"Qß?™0@¤/×?€GÃÔ!Ë?‡Ë6¦ƒ'™?…Šè+=?…=>­mj?ïµà‡È>{?p³§öøD?[TŠxkÚð?P(x¿æQ²?~:™e›Å?mH¯C<|EAGN4FGL J0719.7-4012?æ×$ˆ9dÀ(VȒ«hÏÀ9¾Ò–³5À<ºö
³¸@–R½<6@x+h{?¶é±4v?®ò«â$*Š?öê¹aµý}?÷HýLœeÒ?ëG†Â&€¿ãr
™E¶Ã¿äÑ[ý¬¾¿ß ϧƿäퟫ+'U¿êi>]ˆÇAGNbll3FGL J0720.0-40101RXS J071939.2-401153?w[›?€'ö‡3Ð?Rl¹êÄ?L Úœ¯Ä/?ŠÒ} E®?~Þ¢§P6²?ë`I΢‡K?À‰¿¦¿?''=)¬ Û?'›°cú?;?ÀL± @^·?½ådƒ?îÝnF?æ†?ŽáýñüÀ?€ê>Å\?~Ä›¼è¶?œPÂ8Ç4?‰É$ÞÃ?ëïs7Ø×?Æ¹ê[8?§þ›u°ð?‰Z©94Ø?´…ÚÛùÓ?ˆÇ<…yë?îñ<Zú!š?'ŸÎ"5n?mC^?¥'?aù5>…á©?ž0ÑøÀ"?ôÿUg
÷?çN×øqc?É»ºËîU‰?¢`5ñdÂÞ?¢úSåý—½?Î/ß"²(ÿ?Ȝ븆€?íº–{í0?™÷$ Yv?ŒÃ>óI¨?"§5÷NNÄ?­%ȓ6ü?–
É:rÌä?æ㠚Ãÿã?¢ä5)YJ?¼#‡ÞJ?˜ÃHú?ÆjkÑÛj?{˜.ˆÎAGN4FGL J0720.0-3507¿çþã%ÇÀ#ÈîñºÂßÀ: žóu®À;ýPMö-@ѯJ/ùî@økú$ì?½	§ž•?ˆ1È=à¥?ËnÞÅr»^@©èsFs­¿À"dÌ2s¿äK G2Äx¿éïa|¼¿äž{`sˆ8¿à'ª&¯—2¿Úk	Cº[AGNbcuAT20G J071959-350448?ï·ì)x8:?~'/Aud?FÊÕçeT?BNj:ð‡Û?€˜HA%yã?|‰¸ùË)?ï›ZJ4"?£èmû¯Y?6¿´†Û?N3ŸØ{?›ñ•ég¶h?£®BÂúo?ïV£®N?ŽÏ±¼L¸E?jÚª¬v¡?hÄëFÕen?™YÖ,"U?1±ê"'	?ï滥ªkp?FCËôùÜ?…–ß¡ä?Œï³‹|ä?hH1 °­?E´SÇäh?ïh!ȸÒ*?'BIÚI??S-ås•W?L×ip¼?'Èíԋ0k?¤)X°?íP'½?ºv–Ed?Ek¦?>#?`9ÂÄ`A´?µTÈ,1¿É?º_G	.'?îȄ"£?žfQÈ$?xV·_Óß?t}·[?¬È ËřZ?œ«È!?¶f?ï±cÝu?gÈòk'Ð?;K'u/?*Avïü?'å.b?g$ºf2AGN4FGL J0720.0-6237¿íZâPäìKÀ4¹"åûqüÀ:1SÃÌsÀ<40i@µ—;ÆU@¼›"Ud¶?ÇWèߧðÊ?Ï5E‡Á?ý5Y~ —@›èñƁY?îó‰p"¨¿èyÂÅâοí5#ÞV¿ìÌJ@•òE¿ïÿv}_Ò#¿åÅ2à'AGNbcuPMN J0719-6218?ïÌÎ;{šð?€×‰8(]"?_¥qXMÅ?`Rô–ÚÀ]?q¯…ìÖ?}è¹
LÞ?ïbî|Ÿã¶?•ˆ
ߑé?wp(°›d?ƒ–PA<ˆ?‹ŒLx*hq?Œð9I³äZ?îw0&þ
?ŸÍ$™gp?‰Ù=)žbk?ŠyÊD§çË?§'=²LŸ¿?›¯ê²É'ò?ïv;•Iv?l£
ÔÞwó?{:uØ+s?`îeH»"?"ÓßÂqé?bß0y/ñÔ?ïcºÃ—e?–h÷ !?}ÒÉ"·§¯?€—×Y¼?ˆ'ê»ÜJÕ?'?¬¢¼¬?î4 Ç°ü?±Vn`ê³?"Ò,bR"G?¨fg}'§ã?¢ÌèÿÇñ¨?£:ƃév?첛;ìP‡?§2Ãî.©?—~'Ŏ6†?"

Î^m*?´‹œ/§á§?¤ø£šmb?î5×Zob9?'"
¥¶Ü–?˜0 l!µ^?†í¶iÓ? Šz#ÔèÇ?…»5 AGN4FGL J0721.3-0222?¿ê
¢#	@2Üû:À:ØúåäËÇÀ<b7£Û;û@!
ÂFá'?þ-î \+z?Æÿt>ì$?mWtárÏ?"VdnÆ@[Ž(¢5Ÿ?æþåþ÷í7¿îÏ
)N­ã?ØâõãÇe/¿åQ¯õüpÿ¿Ø©`Ó)ˆ¿À°{±|9AGNbll3FGL J0721.5-02211RXS J072114.5-022047?êò«Ù´7?Èý3v=ãª?c돋çs?oaT¯ä?Ãå¢]ÚÉ?ÈÚÓUìµ?éIþvñ–?À¯ÊÑ}"3?xö¥r¸Ö?'oÿ0?ÊQ7fYâ?À._s» ?í>Ù³KW¨?ž$¡ %?qŋ°äÁ?k™¾y˜2i?´ìÙ¬‹.?ŠëÃí\
?îþeºU7%?y\MÁ#€I?RTã€D=Z?@ÌR
Õbh?Ÿ
úy	Tˆ?xø… …÷q?è*ޗòÇÖ?Ãz}¨*Æ?q«±FÐg?mO²˜¼?ÎÇ(¹CÈ?ÃJõÃ)?ãÀ:{b?Æ2ŽÈ…?p?'-Â#:ü?¯œ…õ1w?ÙKÊ
ƒD?ŗ äÜ[?éSG?®ë‹N´5U?€8C`n?sOŽî¯È?Ê»X	›# ?®xÊQ~j?í	úì+ ?˜/¬qáº]?aý›†Ò?UÀ¡¬ËÃ?· ;È
ÎÄ?˜D6vð³AGN4FGL J0721.3+0405?â×3€`°@!.3ïñ•À8îH[¹d:À;Ö@&t@™`ùj½@}ÝÙdŠÄ?­Ù=ôWUQ?ÀtƮЍ@u–AöD•@à‹†"¿Å.ld'5¥¿äÊf¿ç5ם‹@»¿çÿ©-‹S†¿í¡#›æzô¿ïÿç<t%AGNfsrq3FGL J0721.4+0404PMN J0721+0406?ïŸ—Šm#?w'™PÅ©'?oÅÊPÐåÒ?cܟâ`ÃF?€Kg––÷ª?rßõX½?ïPRõ–è?›þÂD0ý?gœBŠ=?vm­×c?"4†ÇZ?˜¨"6·?ïiS³±Gá?"|®Ò'ì?tOe¢ôè?výIh"
3?‹ƒ`>¦{L?~D-ó€…?ï­£ëhTŽ?`
¼•7?nšê·Lg¢?QtO¶‹<Á?yà"àaQ?Vã"G˜ˆ?ï`­Y6t~?…Nà©F·?y†úµ3®?r܏ϳ—?‹,ùÂÓ?>ܬ
Vè?îGjÂcÛ?±ÊÏúš3Ÿ?~:¶	W?"e!uy1x?§Âfg?°jçÆ^"×?ïº Äú?3LÚ;Z?~;?K»Yy?¾Òvw†?•yðßa?Š( }Ñv‡?ï3¿s"c?}ÈÎOت,?ƒéžÆ%}?p}FGz!‹?&"VÄæW?tI1CÝiAGN4FGL J0721.9+7120?롆¬SP@<»à~íÀ6CÀ:Ð{?;2@e°Ñn?ÿÇ@ÿ¤?'AçÅ?­ÄÑ<w•@"¿U›=È@§6ÀÁ&¿¹.CŠCeZ¿Û3ÀîÈ¿âJ'Û¿à£W±—½¿å›aðµà¿ä1Ÿµ<OAGNBLL3FGL J0721.9+7120S5 0716+71?ïÈíu‹?vbñ`GN?T`âX¦:Œ?VF­HVÁ?vqÕ¡í±?sqÁ¹H`—?ïTƒ]ÿì?£%F±KYH?lyz	?zd¬Ž$+À?'àdP®æ?¡ÕÁҘŸ¼?îº5ð@´?œÐL8[ÉÒ?'Åï¹7ûä?ŠXj±A•?ŸVJ-÷"?˜ºµ
GÞd?ïâH·©Ïó?Y!Ž"?H³‹™PÉ?@Ô=YŸø?gŠdâ˙H?TÀIKêä?ï"	«‹šº?‡7%7i%?[ƚs'?^"›N·µo?‡ÄÁ̤Å?†'×ëvÍ?îsÃ@?µFƒãàö·?"MDô-?¢úÔk(w?£»"æÎÂ?¯Z0€®ï ?î¾tü›
w?ž4Âô>¨H?~jÎkì?ˆ-7(‡Ê? K`íÑ?›vÐÖl"Æ?ïÃÆ=çl5?r[Ÿ?U¨+úMD?S¢¯Ûåðe?x²Õð)û©?pu?
Ü2ƒAGN4FGL J0722.7+3606?ïð×uÆE@5ZÀ?öÀ:¤p¼*¾À<xåÈFUO@æ‡ÒǸ'@ـõ]åŽ?Åã!wôÙ0?¸ÔÈnÄ-í?ðdåÈFUO@º8	0Ö?ï—ùá­Ún¿Þ—¥ãÿÄF¿é¿8ÇǪ¿á)Œ 4Rî¿ïý
í™Ëï¿àIí>²B]AGNbcuMG2 J072255+3606?ï¿tO¿‰?rf0ØÝH½?aOæ¤¯Ô?YÊy¸_ Ý?wäü÷;{?lº¿€G[ß?ï¬ð
à?€³•O§B?d6£îÊ?oq¢³À ?l¤aªZ(?u'L0JÄ¡?ï]W·³?'ËëþLÀÞ?té{˧°?vƒ	teˆ?Ž˜uXüÙK?{£oy;?ïŠNÐâJ?b¯øAvî ?yÞÕèDAŒ?Xº—¼,ë?€ŒH‡Ð?XI1(ïEô?ïŠ7!W?ƒŒS§É:x?p•2™gÀ
?i=Ä8®7?…4Ü%øf?d"âÆë?ï{÷V£?—i^·r&÷?v¹¾'ÎT†?€Órø»?–ÂsJ‹?'N¶PÇ^G?îÄè‰/­Ü?óÐQ#¤™?€û]€Ò	
?€z<ˆ!Ç-?žå@Ћæ?‰JۖJL?î¯Ì!"²?Í‹ãÊQŠ?'Dýš{êþ?wüSÇÙ+?—×èڀ†Ñ?xÍîzd}AGN4FGL J0723.0-0732¿ïSò"äVŠ@_9K{)À9äٞlg1À<±KgŸ@,­†¶h@°››ÒXþ?ºu…NQ?¡£0P¾^?èÍm¦Ìˆ@º	Å{ ?ï‰>½ªðÚ¿á{0f…p¿åÅ$aß¿áKñpD¿àÈ.3ïò¿Ù¬¾Å"3‡AGNbll3FGL J0723.2-07281RXS J072259.5-073131?íôf'%ú?¢ƒ].c¨Œ?tÿ{$v?e+˜XíP?²°eL\†?¡·JjV?é£%LH` ?¹{k\ú"Í?€›bXz'?'mW
Yb?Èi´¨Øjª?¸d…::?íÒ­ˆ¨Ÿ`?•ÊV	}Öe?ƒ"î@Ôø?{Fkè
'?­ô$vú)Ê?"$Ě/Þ?íë"8º9U?€¡õa'-?€s¥Ã2ï?YcÝTQÊ?­)ûõ(p?€v;÷úm?éäÂè‰y?²™´'T—*?ŠÚ¥W±Ðo?y–ŠéÑ?Æ¿J
î¤?±Ø'âGÊ?â=&:§i?ÆYê­‹?ˆ³;7UÛ?³2O#¹?ÚÀ±¾Õ?Å»­q#?êuÙ4±…?©H=*W?'sæþkg?'¶ÐŽ†Áª?ÃÝcÚM>?§Ý€a)à?êG³]î{Q?œXʪ/T\?–£$—?ö?zX§ËÞRÃ?Ä >#|0þ?šêMºh´.AGN4FGL J0723.4+5841?ÛÙi=[U;@:ÿyB=À;å¼i¨:FÀ=¾@Bo@"{é~^TÊ?í@*ýڋÒ?àfQÒ[?æÝñLÞÕä@È¡#і`@a«ã=?ïÿõÿ 1#¿ç²›"nÝ-¿ïÿÝÀåãÊ?ïý¸Ý¬˜û¿ÁSIÔ	'¿Ø=ª]yAGNbllRX J0723.2+5841?í×MH?¯®ëGX¦'?j­ÆΎI?qdMg³Œ?£ıڴë?®×$Oѵ¦?ïj3LUž?˜ƒ®åtþ?pjG¡F7¥?‡¹=hJ?>	!¨ ?"6/x#äG?íñŧêjB?œ¡‹Œ†N?#{tvÇ?"ÿº/È6é?¬šÆ¥¢X³?šÅª"¸£?ï]5ðÒ»y?äþBÛU?U±*‡[‰?SÛÅÀÒô?'þ/>ˆ±'?Âð¡Y~¼?îbÿ!;l›?ª¼{‰ÍÄ{?~NMÄ?†²Ÿ÷m•?¦K¤«?¨n"÷•'?î§ip(~q?­'t"ó	?€‹—t7¡¸?'®û3E/h?¡fƒ >5†?¨2FlS˜â?íB[†RX×? §Ô•¥
"?€áòÊ÷ƒY?ƒñg]ʝ?³Ðåv)™?Ÿf"8Õª.?îœya°?¢
Âgq"?s³ÔnE?â5´«ºw?­ŽoÁoPº?¡_xãfAGN4FGL J0723.5+2900?â
lÿ@3AƒÆÉ}À:¡4êÃWÙÀ<h"»@}¾ýVW{@iüp?Ð#þA¹Þ³?ÁfbÍT²?ñk:á}^@
¤ý·PcÆ?îáßeUÅ¿ãô®ÞOV*¿ãôC¾ñ—Ý¿ê~è=k›Z¿ïõÉ{´Ú¿ïþI¡ßŽEAGNfsrq3FGL J0724.1+2857GB6 J0723+2859?ïîÞ¹%?UQ$ò÷?@·cÁ?4*aY*Æ¥?Z@ï!¡?Spü‡œŒ?ïÙuvâ?t<ºÑ‰â?J<O 
¥	?WÌî""?p,»'
sy?oú8©z?ï'ÂÚ}?|ð(¹X?dO«6(ù?iÕ
=¡:i?†;'¦Ò«ù?z-tcÉbé?ïÕÏѼ?Pz>/?TÔ­ü.£?6/yYô8}?pHl±&N®?LŠ…@¥nZ?ïÙõ½³w?g-UWY0?Oæ^%	B?Gy^šq&?nO÷ü³À?e/.¢?ïŠg'M‰?Œ7ýÕ?`.b"?m"xA?‰b/;ñ?ˆ`퇀³?ï-1¢4?ˆ»‹_XÐÞ?q#lé"È÷?rüÈJ?–ð…g??…ïnÚ —\?†Žœ]?kË.þñÓ?d¦û1Ñ?P84강.?…l—­Lœ?iq¨›ãstAGN4FGL J0723.7+2050¿ì@½È«ˆ@07!-w1À:Zڀêv+À<c" ³Ô®@ £ˆ6šÆÀ?ÿkªs±?¹*Â÷6ð¿¡xô2—Vô?ç:ê _@ü°­\o¿ä›?î¿åôi"PY¿âA¥¼½‹¿ÙɱÅ	‰ì¿ãêÿ½ºá?sKç¢ËAGNbll3FGL J0723.7+2050GB6 J0723+2051?ï´LŠ"h?¦lx­ž…Ó?Y˜›f©$?u¼Ã(¬ò?'€oÅî?£ºŸOphŽ?÷ Ù?…ÂX9-òL?\æÜ`p/¡?aT@Á]¥D?†A¦´!i¹?ƒMÅrè¤?ïwO5ƒ€º?wm£°"Á?dâdH‡ãÏ?gÏ@ò®?Œó™'ÍL˜?rÙ-ëb"?ï
'þˆÂÃ?w[ëÁ8S?j
®º<?LÒÖÙÞÏ?šýþqUDå?wO›¡Ä#ô?þc?Ë_‹í
Ô?b†C,{¹?pëð {a?…=o£Ü%¡?™ª¶L'º…?îۈ[¦m?Ÿ¸n 8'?p
îöXdƒ?{ðÏky©ò? E¼cþ?&?œ¶;0š·?îã~<'#?Šÿò-YU?o&øÅ'¬·?fWsÔÂöC?Ÿ·ñFÕ?‰¸™Ìà¼ð?ìÿHÍÇÏ?"ÌÜe•2?"'YŽÞ?oØ2}¡™?µ…²¬o?"Ò"ûlBUAGN4FGL J0725.2+1425¿ë"àD±á@+Ó"Àh¡À7ÝàÇU•À;‰¢TS>k@4#.XX@ —Œ™?—ÄCøc®?°²œøž¸@AbÙ,@¬¸ú²ä¿Å"V¼OQ¿áfÕÂ>ÔQ¿äËj—MŽÿ¿ä
оsæe(]í!¿íƒá¡p'°AGNFSRQ3FGL J0725.2+14254C +14.23?ïÓø@ µ
?p0 Ò#"?Gl´ÐBm¿?HT.ª'-?sI6'J?l™:4j|?ïÓ¸Tš·?ƒDþlêF?Gâ†ÁŽŽ?Z«w,Ô>Ç?s|RÜOÝr?'‡—"Kù?ï¢)Ññµ÷?ƒ	™xê¨?eü–œ?¸f?s5Ýóßp?öeØ»K?€Ñ3u'?ïü
Á5P*?'·–>¤5>?''ìÑ>ýDLë®Ø?<)c
ˆªÜ?%ô,`ú'?ï¨xãP?ƒµbÂ~Õr?@uÏ0' ?@f&	‡ó¿?"ÚjEùFn?ƒ>ò]MŒ?ï—îêë'?'‰
a:Î?Qækœj¶+?c)U‹c%2?‡ÇwÏú'?Ô4ò'\¨?ï'bŸB·?ˆ€tqWá?fzÆPÎýé?uPÏožY?†¦Ï¥Ø?"ó®6Tgñ?ï÷)yù\?EsÉ*Ԑ?—[\Fâ?&]Ìh[?O—ÉÉz¥?D:²æFnAGN4FGL J0725.5+0216?ØÄÅ䝛S@!AlÅûø4À9Ò¹
x)À<ñü1>f@
Â
|?ÿ1³¡'œ'?ºÇð-"£?³¡ö4z0?úqºÝ¶ÿÜ@ÑîøEÌh¿àã£=‡J¿Æ(G‡S¿ßøÔ<­°R¿áAn?"՘¿Ü/0Åпæ%Pò`ÛAGNbcuNVSS J072534+021645?íD†'B÷»?Ŧ€>Ì?xèG§ágX?‹ëíoE?´MFüž°?ÄJÚCØÈ?î¦ZÀžsÒ?©	¹øjҊ?V³sÌŠ?cøÀÙw?¤ä¸_")X?¨MìòÏ?ïÊ_¸Ú?­ZD-Ò,?còýÀå?Zt"+g¡?›TgMå?Œñçü?ï`ú\/´V?d¬¡µÒ]?c-™Îð(ø?@À?¾ÔÑ?'{C›?c¯÷ûð'?ín¸lÃw¹?³ªP Ÿï?xôc/ d¹?}3L""D?²úögç'?²%€F
4Ú?ìêL"O¥&?»°¸€JÏ?jÌÉ¿u¥?'"}w"?·Üäøáª_?º$Ÿéâ(Ì?îX±
é,?š­Uî\1?r«êò*>?kÍ";?¬T÷œ‰"?™²ü}OÈ&?îm
Êw?'ÑSƒ+ŒT?uè•å3è¼?\C	m{©P?¦rÝ@ƒ?'A_;éÖïAGN4FGL J0725.5-0504?½ ˆK=–@í:>À/0À:Û_D35·À<BxÔ'4!@!THÈpǓ?ÿ¯®(œ×<?Ãs…]Íf¿Ÿ¯¹|Ê?ßÿ^¢Í @aW<|Þ?ïõub'¬¿ár"›R×=¿ë*:э%î¿Ò¹'"µí¿åµ(€Ò£P?™òåæ#`AGNbcuNVSS J072529-050338?ëƒ6$n
>?µù]øµ‡?kÓ
æ•ô:?`{à½AÙÝ?ÁƒÛ6œõ?µíK¸ß0Ý?å¢ûØ~ê?ÀñX×:B?‰Nß#¥£?‰Ó©8\¸Ÿ?Óï'UÛÝ??À–"»è"?íÕmt?žÚÉˈë?xۑ¬ª^?jÔ_	6;?µ°öÙ?ë¶?ž:süù{²?íX	5!¹¨?'ý!©
?€#…^*Û?dÌé‡bF?³;E«çÂ?":ÛCB?æ¯iªò/?Â;¹Ûi®Ö?|"ïЩ?pë‹ç³?Ò.ÜîT­?Â*mß#?ÚÖü'Рä?Äá¨åD›n?[o΀<b?–6A…†g?â,˜öm?ÄÉH-ãŠ?ééh 
¸?¬Â'¨¯·?"6Š£­ÿ¸?w׃=nkà?ÊDñ²Æw"?¬@z3"ÿ?çÉæòyû?©_¨pÇÊL?™‰¥àòn?‰@h¿ Ù?ͧ/y•BG?©µË86MIXED4FGL J0725.6-3530¿ïª>°tÎÀ"gn¤"ŠÀ:Åõ´L£GÀ<!6ãÁÛØ@ 0Î"oO@Ãlß&k¥?Äí&ο ÏÉ£Äã?à'qßÁ@Fx	|?ê'ݝ'A¿èæT]Of¿êýÑb]ÿ΁¼ÙÏ|¿à'8¾né¿à:Ã_æš~AGNbcu3FGL J0725.8-3532NVSS J072547-353039?íþ`ºtí?¥k9ԟðo?bw-"(?Y»‹IëM?®ò"@²?¤õǜ%(ó?莯"´…â?ä¡Eƚ?jç…^Èé?{E<D³Ê?ÍY£›ŒI5?­-÷Mï?íÜUJ¬˜ò?œ:ˆ™ú?l"ŠÛ‡?cʬ ƒÓ?°8µÅ.™?›ñÒíW™µ?ï5gÛ'û¿?t÷ßµ³±Ã?N"ül(ó?4}î6a¸m?˜^kθ½Õ?tç3JÃe?ë9äÎÝYs?·
S†­H?vQÅËøа?oPÇ8ÓL?Âeޖ£Åí?¶  }Â?â1[i?ÆìÁ´À¼s?gJ²G¼µY?yÑXE9º?ÛÉåkmü?ÆÔûþ¥?êñDñþœ?¬îtòƒ0E?|¹W©"b?tÒSœ	?ÃU%>†?¬R6,ݏ°?í+Ý@¸Vô?•ÙDY•*q?l#lέË?[Ù^±^Wß?µ¿ú"¹¾†?•°Øš
AGN4FGL J0725.8-0054¿ã&w9-¯L@ñµ ÝDÀ9@†ºŸ¤À;ûbqåª@k¶ÓfD@£ì¤©(?©¡ÛÝ`î­¿"Fù¨fÕ¼?ê':…7@–¢n5é¿áaÂÈg¿áµ2Ùà¿âíp3Sê¿ÜŠÛ»¨N¿á%_Ö)lá¿Ý×_¢ÒÓLAGNbcu3FGL J0725.8-0054PKS 0723-008?ï8Kݒ܀?Žgý‰:ù<?XKd*j˜j?P·zR?—qÎ걈?ŒË5©ø9ø?îÛôºsü?¤ËF/{?Sl(°?b'"uÈÃü?¡§÷ØΔ¡?¤1ÿ
‰!õ?ï#'hš?©?†ÿö}œÏ3?gQ¬L§?a•*k-áh?˜£}e^é?…ÀìbÌû\?ï‡ÂéÁqœ?e£û¨›Ï?aP?€š?@pRÓK·?‰Ê€õ¼bÐ?c™%9¥/%?í¦‡"kV?¦løœv}?of
¿¿ã?dJƒyw0R?±Ð–š—?¥?êE–}©?ìo ¼¹l?¾®þ?gø=O'Õ?EÖ+£Ð?»Ç8/¾«ï?½hMÔ¸Æ?î)
ы	?˜ÉíÞæ?tµ+Kt©?kæ¿K¶¶?­6ËaErÙ?—=
›Î?îÒRÂrè?"Oª?vw=´ûy¥?^Ïâ>˜¨î? ÷ë?›Ð?'}žÌqAGN4FGL J0726.1+8114?æ––b‹@<ÊÙ­…àÀ;çè:ç\›À=#Èb±@!r˜k?ûkëšî-?Ô)|»'gÌ?Äseè½O?ð<÷ØQì@‹cöÊw¿ïÿÿ)@k*?ïÿˆ¬Œ%?¬,©ßÀx¿Ú"s,G†§¿éôœßõ¤?ވ^Þ²¨^AGNbcuWN B0716.0+8119?ïl—ôå?˜,lR`5z?`ƒW…œeh?[2*m'¿?n"
<W?—‡® ¸?ï« *¾€À?€úÁPm?\Ñ6R<Ù?d5>–·¾¨?}Ίۜd?zµ¢Ký'?îXÒ§WGe?™~·Õ"¨‹?…«¿ÂëP?ˆö9ù8?¥å˜ôη?—=G¨Ó?ïd»~ÏF'?túî³é?rËÐä4L?ZÞç‰×È?ksŠy1?rÌÎÞ í?îD.¸F¥M?°ªGaë?v¦É)íuÍ?q}ð~×CB?¨è;R¼ev?°tà{²&?ï?~½lª?—Îô˜ŽnÓ?o9ãáôI¼?|›8ÑêÛ6?™0Ó¤°¸•?"¾ÖÁ¢Š?í±ÚÑ0+?žÍßÇPa?"µˆø˜h?"µ³}0Ýa?¯´ü©6Ú-?œ°ÀhØ?îs½ã¡Î?Ãk1ù¸˜?Á¢ƒ?u´yÛju?¤Ë틫'¶?8²rÕ÷AGN4FGL J0726.4-4727¿Çú"«uå
À,J ÊæBÀÀ9$ü!N.aÀ;ÂÁÀ)P[@T!¾@Âé@?Ä;-Ó?°s‡Ù~?¿úš ¹D@@a~ @Xj1Ϳ΋ÜÁ¸r¿ä•¤ýzꂿåÍùƸ¿çŏc}(¿ë—à±Ü¿ïÿÿ" 5•AGNfsrq3FGL J0726.6-4727PMN J0726-4728?ïèÓŒ)?ZîûêªTé?H5'°e‰¥??Ï¿9?ažeb-½?VÜÝ*ô6?ïæMå:‹?p½¼¼Cõœ?8Qû˜ÎÝ?DÊЄ¾äÆ?f§ÛK¡±D?niè&q/?ïÀ4/~ë?yŸ¹ŠÏù?gyç,^?fØ$Ö¹?'Ï+×R#?v›çŽ,p§?ﱗ¤nVA?^ýJ«ŽPs?Z'[B{•?=ãTöXN?€Iˈ!Ÿ©?[œXb?ï̦ã?f.?k.›hå"`?WY±ZT,!?P@éLç™q?sÖ"*´þ?h?ój6?ï¾æ%u?'¦õºCñ?PL)Œòx?^¡s½oí8?|äµÀügû?€àž+rÌ0?ïmfó1?""q #—ý?pP'VÑ^?rš2
 ?Œ¥›g!'?€§/%$Ü<?ï,•d?{íވ•Ÿ?r£RÚX#?[çɊp"i?•ÖÓ×ø}?xïN=ò¢AGN4FGL J0727.1+3734?ڟåtIº@6Êÿ:Þ"`À;Á­!5Ú­À<é°¤xí@!À?ÒþÀ?×fxÚÝ0È?èùäÝå£Þ?ïûÙ_'F—@~†T@wUCÿ3Q¿ë?.Ö­ ¿ë¹‹§i¿Ð'4è¿ÙcÍÚ¾Òä?¾°»Ê²¿ïÿýFKêAGNbllSDSS J072659.51+373423.0?îð
É©ú?²ˆ®i…?w4(¹‰?…ÓW3'ª?œ1¡ˆ‡jÆ?°É¯¶"?îö6FIKµ?¨mÖ»@»å?w304úS[?‡Eš>G?›lk/›EŽ?¦%¬‰ÅÃ?í»ÌÌå!?¡CS8w›?…%µUF?…ƒÀý&U?®ûtџU¬? Xì³Ð…?íÀÖI^?¨³»ñ!?Cº>É¢‹?G¶•gKÜú?±ØLÐƵ?·
1çl?î4†?ª«!€~ µ?‡Ë°ì<@Ý?ŒZ™cÔ?¦Ë+YlzI?§šÿòª\)?í¹Ã•8r?ºž=$E&?Š}!û£?Ÿ¨ÕÕ<»{?­Þ'KËï?¸\ÇÓª?ìNfF	?©EÙL8È?†‹¡š€/¡?††X›=?º»[º²?¨!æñv?ë–f1?ñ?±Ä@ù¼¼V??#¤Yè'?YcÃþ­Ô"?Á–ã©)¦å?±ÆR¿}tnAGN4FGL J0727.4+5325?çŽÈw@:²v‰ÊÀ:íâXOLÀ<˜V>Ðö'@'èZÔ@ïd†'V?ÊJàc'†X?ÄO3Cú*Ô?õˀœ?üåàaª¿â Aåþw¿æ½£Ï}5¿çFÓ#(¿æ~'bEo¿ìmå€ø¸ä¿ïÙuQ»´wAGNbcuGB6 J0728+5325?ïT5år¾—?‡Ì
ƒ\X€?zNÒByï?ppJSë³?£ßI¥[1?ƒ¸	7‰s¥?ï)Cÿše®?"<Žaé:?€'™ô«­?R/Ÿf?'Ž3öú?‰cæ7	µ?îԄ£à'È?'IøÜ(½?~C¾Ôc/?yá>$¦>?Ì"8®3?ڋ§=œ?îØÎôL÷?yÃ!Âcb‰?ÒI÷5z?pv†àÕ{q?•\¸J†Le?q3ý€«?îFbð°? HÉUg?azã-ß?'Ú`êƒÈ?¤S¸Ÿ$e>?œPŸʾ?í›ÚåÜ?¨s>cƒ+?–\Ü+sþ?˜Í'úë"?«Nӎ<?¡…¹j~ÕÇ?í'{@Ï9J? N A»w•?Œãªª{"½?ƒÓWtä ?¯¯aD"¹?S9Þª1?ìÎîN§®?—qþòz?¤<eSºê?‹N¾­cö¬?®â!¹1f4?lê!
VAGN4FGL J0728.0+6735¿êsHìáL@<e#'Õ€À:D6•¾BÆÀ<vî>6œt@38¬nÞZ@ñÈ`2p?¾š%@èc½?«Ÿ!ÃÊ¿?æ†DhÜ
@`«fuªÒ?ïV*
ðƒ‹¿è…H©¼ýL¿ë&àtI}ø¿íecœ‡Š£¿ïÿž{€©ß¿ïÿÿÊPËAGNbcuNVSS J072854+673225?ï¼á½þ0{?kC¢?rE»)nÛ?}Í¢vÁ?n'Ëá͵_?iÎS0Øá?ïH¬"é£À?"ä*·ÿô?Üó,'?…Mð<­I>?ŽTmìíÏ?†>ä=íü?ï›ex«?}òZa1?{˜9¿Fõ?}‰9á‹?˜fÊñ|ñ?‹à0·ð ?ï[¶†Ër?uýތť+?Š*Sˆ	Æ ?r	ôÞ¬N?~ }'	Ùò?aõË)BÉ?ïŠ3+›‡?ŠXoO:,?'/Z"$á?…˜žá›Õ£?vˆX¡PK?x~±s?î"¦{²Üi?«Qo}I(~?'ր܇¡?œÑ'Ì~oÞ?¥L-ˆœ?¢KBSϚc?îÄ%UÇT?—d¾ ®©?‰\ˆ
¢w[?…èTO©Ç?§¼›¦_ç?"ÚO—Aûx?í ¯˜½_?œ‰ëÎ0)\?©ìьë"u?™†iL[ ?˜iÑø';?Ã=ùh¬AGN4FGL J0728.2+4827?ïòQs»
³@9Òe8hýÀ:´w
}—À< ÝÆT@Ÿ1ƒZ¾@'Ê<ϔ'?Ã;äI·¯?±êÄÚe?î5r£‹‹@yþô'9¿âwÉЙ
(¿æÂ
÷9‡á¿ÜZ›âŸ¿ä &æô–?¿ãø?"û'¿ïô ÞÇÌAGNbll3FGL J0728.0+4828GB6 J0727+4827?ï"ÚAgð?µœ†¦3?Y‹Ì]Ï´?ƒôƒ3ݚ?‹˜ù#.?´8M'gÎ?ïÇSk{'?u͗¨Ë?Nà##c?R™Ñµ]·?x"gä0dÎ?rzàl?ï`>å+
?'ÅI,?sÍâ è?zžÁ«—W$?Ž`'¾"a?y.•†H\?ï'Ëžhý?fUÁšÂù	?k7~‹ÔØ?K©iönct?ˆ8Ø)Eu?d¢%sÊڇ?à¯WÇ?†G§'' f?`êëðû<Ž?UŸ-2åCà?‹cŒèi?…Q™ýL?ïaŽm+Û?Œt3
'Š?bqùüŠœ}?j³°Ýìð?'ýø}?ˆ¬<±h?îíàŸ"Ö«?ŠA^@¾fL?y=ø¯6ãd?yâ»5Ï?›ômøÁ?…XŠcNa•?î°:ÄGS?ƒ?
¼–?€:b´Ô?háϏ1"B? íÜ_8‹?ÈX	œ[AGN4FGL J0728.5+6128¿Ô0w@;ûd¾ÆyÌÀ:b]¶ŠkÀ<üýíI@%DĀ"$@\»‡*+?Ãe4b2O3?Ä´ú<ü¶?ýR;×F£R?ÿ®B0èU¿àtéa#q¿áÌ{n5gÁ¿éޠ4¿é'Öt{'¿ïï{ÎRß¿è!^™HAGNbcuGB6 J0729+6129?ïƒh‰+§?õ÷G…‰Ç?v~
:êÑ^?pU—"ìu?ƒæùO]õw?uÚ¹ÌvZ	?í§Ÿ>»?°~ÿQ"Í?¢E€•ñà?¤¯Hjm€8?£@Ž¦Ñ"z?œ;7«Œ?îÉåe¹²?âm5k?…Ѻ\¿?¢‰¡6Ãw?›Úv?‰ž}e"Çë?îd-ë0÷*?…zÜhkç?Ÿ®ôV¶?€gæ¹
ç?"ËN¹Z?q ¾AfÎ%?îçÎv×3?"^x¨T?†çòOå±Ð?€'a÷ØÈe?—'7þޒ©?/÷†¸*#?é÷0*6¬²?Ã1![Ö{³?¶Ö×ÖÎÎ?»Žâd]˜?¹o¦Ùð!?±Ìu;¥Ï[?í…H$˜!?œ}t8ÐÅÅ?™l`:"FÄ?ô䕁·?ªõMšH³Q?–
ß4Ûb?ë¦Þ§nY?¢dêŽt?µDŒÖJv‡?ž±¶¹š\?«ûåÉe?…"ÉkŠAGN4FGL J0729.1-3131?ïðѱôÀ<¹½üOqÀ:CTY©À<Wۉ(2@RG[^JŽ@À'¢Ü?ɸàœ7ƒ¥?¾JÍْ-?ðEUDÖ@JSÆP±É¿æ-z¿âp Ñò&¿æQøàüڇ¿ÝÝç;ãÛÝ¿ïþ¸Ø#B$?ïזàÜAGNbcu3FGL J0729.5-3127NVSS J072922-313128?ìß2žD?«ë€ûf^?'þ{Ò +?~‹?
"ìo?¶§ü`à«×?ª_aßIûA?êWåv*Ãg?¼žüM ¢À?n#ß¢?u«÷ö·N?Æ(™&úb?¼ͅ%æ'?ìs¿cò\˜?¢‡u(ñÇË?'6e×E,Í?‡{ŽÃ\?·ÔkiQõŽ? ^éX>r'?ï	'·C½^?}ìÝ[3Ü?nhV	vQ?V¯	µ6áD?›žWþËv?{!Ê¯}?èX
wʉH?¼veïÀd+?›ÒþN«Ýà?š^,lUÏÑ?Ë%vWÜF#?»8[YJ§¢?ã3Òåbd?ɞkXœ+ù? ¼øãé?ßZlRљ?ÙÙÒf67?Ér챙•"?çfŠ!Ù­?°˜=+J)Ç?¢"†Á?'ø$Ù!É?ÍÀµõ[ê?¯€UÒyÇÞ?í/·ð
®I?™ï­¥ç?ƒ•Í®µdÅ?t!;—ŽZ)?´†É.óä?˜:›kݜôAGN4FGL J0729.1+5703¿ïì|™ÈWa@;'ýq?À:¶nÒE²'À<—…\˲ñ@V±<£@ƒ¥An?ĝ•½ ~?¸Ø›ž<Òª?ñvÙ*© ö@ïéW•?ï¼ÊUú˜¿ÑÛiþKtó¿ê=7˜ól¿ßJ(B>hñ¿í­ÞA¿=¿ïø#'¬?AGNfsrqTXS 0724+571?ïÆnÁ
?£OU¬?Sƒ+èò¸?Qçò¯8S?wçÑÌðò?£O½TA-?ïØÔg Î?qøÎ&èÅ?H¨,0Š?S&6|¿i?p€ÆÎ(í?mG˜°9"?ï…Nßó+l?ƒœ—
ïË?iÞÚ3O—?s¨€1©ž\?ˆ4'ƒÕÊé?*¼‡è'?ïÏmðb‡?RñC?•û(?`"Æ
Oz»?A¨@™F©?oþ3½•Îé?N¬3šT?ïÍÑùÇ?qò¯cö¬?`FµµpÈ?_<.ïS¢Ñ?pô'¶§?ld¥ƒ¡!†?»¿ß?"'ñ—"?WÑèÕhë
?a<ÓÞ¢Ü?ˆ˜Ÿ"ÑFÀ?'0ñÕ9ì­?ï:'1E?ŒÂ;@¡D"?r+{0[h5?v'°U@L?""ÝÕ§Ÿ"?‰(ZÁjå?ïmKò¿,?tœ›L¼7$?y´<BV?e0¬Ÿ°?‡Ó*ˆ¥è?n"'á02(AGN4FGL J0730.1+6852¿å*ÆR4U@<¢5¤À;ôrKvö×À=x,æ0@`ú'ùÄ'@6âÔv?Ö&DÉ^?íâþ1ɦ¨@u-fj˜$@~=F\…½¿ï÷Ìàméh?ì¦-['Ý•?ÏÝê@ûó¬¿äîÝ}I,¿ïe©!ÌÙb¿ðAGNbcuNVSS J072949+685305?ê)3"ñ?ÇmÔü"†R?¶*¶hہ^?¹²IW¦žÕ?¸Œ¿ú(?¼·~qu
H?áݙx.p?Ê]i·š?Õے¼Ÿqå?ÈÙ+xv?¹¤éLî?²eŸ˜Áj?èe	µi?°ã¡D–"?¼à?	D??¦¾6w"s?¿÷sKs"B?¦ó‡C_¯?æ=¼ðÐ{ó?®úwBM?Ñ|ëÒ»=?«É:=ŠòY? <ÒWü?½żÄ?çh3?Èlì?ÄÀ{fÙ?ÂÒޚæ±á?ºFÊ#"?¿¨Ëï4ß?¸Á¬ÒM»?ÙØç—ÿ:³?ÍOy¡ö?Ý9(ö?ͦ$JÔ¬?ÁÛßÓÿ_á?µéÎӔ?ãþŽj³Êj?¶c]PÓ?žÜÙ#6*?°²cít¾í?ÊFéyçÞ²?°aî-UßÂ?ÚX%Cdv?¹¨h`Þßk?à‹_R²Ã?¹8҈ON°?²Dp^).Œ?¢Wv~Iw'MIXED4FGL J0730.3-1141¿jfMfQ@	ì:P]æÀ6ÂôÐ÷Ô¸À:ïø»h {@ÓÑ3¹ÀÖ@ ŽÉ[ÿ?ŒS¹Vç?·5Ed8@'€2¹¯æ@ç÷¤'Å:¿¾>Ž;Ô¿àñKÞ'ñ¿äÞDÄU/¿ä"BO/èü¿è=N	xNÆ¿ë÷ãœ*ÙAGNfsrq3FGL J0730.2-1141PKS 0727-11?ïY¦g2i4?_\øM?YXœ˜ŠM?V
ù$0a?"5±µºÛ?Ž~·ßã|}?íe7	V•ä?Â@Ò"š_?~X¤ì'î¿?'ðÚej?²ð½fÚ'õ?Á§ÝßJÜ?î·òšfÉ?›)jlj7?Ž|œ°Oi?'èây~¾?™Þ¹W{Ç4?–ÿ7+?ï/ºù?|
3Q'w?nø"£¢¸Ð?fÙOKöƒ??"õðFIq€?sA¥•éõF?î&¿·1ýK?¢Ì8êa›?kHr§Ìh?gfeª"œ?«ß}c	
?¢r›<¬»?ë0ZÓ¯s?Ê2ÁŠñ­y?'Ó•‰T?­²HIœ‹?Àä7w…I?È°º<ÒCY?îDT†üR?žÈ󃭺‡?ç÷È|?søÆûp?£r×Éÿ¡?šªøŸ`t?îÒ}Rˆ…m?"[bs?Ö½óµS½?z¤Z–
±?œÄö¼ۇ?ÍÍÙ5AGN4FGL J0730.4+3308¿ëë0CÙbv@6NÆ6°–À:D¿Z'ÈÀ<mÆ	d-@æu27}?ýˆßØBKÕ?ÀA«›úœê?½T›bÇuu?ýƒ«kS51?ü8ÀA¤¿ï{œŽ@ ?ïñ¾>¶ì¿Ý!_€îýÏ¿Ô É°·¿ä´êÓ¿åÀ_–¾sAGNbll3FGL J0730.5+33071RXS J073026.0+330727?ïÒ5ñ?mӝ҈€q?QvóÐêb8?EF7#–»[?yÙ(›Ä²ó?j'þ¤¨è?ï0š"7ÒL?œ¸îuHil?'D533£?¥Oî?Ê©]¼0¹?§g	9ê¦?ïT<xl·?Õ¤óîè?k™FÙrhx?fc^Pn?'H$˜!?|‹4²RbÏ?íH‹ͽ?†ª"uBC¿? ì£q}©v?zÂQwzJ?ª'câ€ý¼?€¥8ª*£?ï–QYJ/_?vf5Þà~?aïÀóÙf?Q–rÕË?…ï¹z¤OÅ?t_ù">«?íЎ"ö'±?­S°víא?–ù­ÏU?¡šénÑÁ?§ë ÷¸D?¡Çìò"Ú?îÆgýâÑ?…•FFâó?xEáßw*?tŒ°×dˆ? Ãé±,?‹"ɛ¤g§?êkÃkß1?žG´¦c¢)?°L#4¯_?ÂÝTE?¼UÁŽ¼W?—wz^5­pAGN4FGL J0730.5-0535¿é"¡]:÷@Xr)é–À9C_V§¬'À;û[Ð
nï@Oªú•@(šE'É?±ŸÑÛÄ?°ë	_
´@~%ŸÌ¹'@º'
ÛÑ"?ïîè¶7_¿ãDêJŒM¿ãI"â s¨¿à{ÿõï¿èiýà)¿ã,+6åo[AGNbll3FGL J0730.5-0537TXS 0728-054?ï¹2zéo?lƒaž›V?GÀÅã?9eS^fÄ?€AܗÂë?kÚP3?îåÙI?¦¨îɒS×?Z] –X?i}ή?–2?¥]»Ë^?¥Õ-…©Š™?ï?‰Hh¥?›p–cÌ?fÌì"ܱ?T‰HNƒ]?•Bñ<#äå?€"¨1@£Œ?ŒÈáí?fQx"?k´RÉ£¼ü?I'UKá%Ü?ˆ2Höۏ?cŠmf"½w?ïA©}ñ?'uŠ§«"?^¨¶#Y«?Uæ†V Á?•àQ'ԟ?Žð¥Æ­áÁ?ìÐyêt?¸QaÞ¸™?qVkn{oJ?ˆôÂO¿]?¸fÉõ˜M2?·¹7²#?î­¼T•¿¬?'xÁj•‹r?s)cXñZ	?jêžk{Ô+?¢¿JÕî?zòm"ö®?î·§5'mò?"'窐æ+?ƒ1èvF¼Q?iWrÚ÷^?Ÿr%%BH"?xâxtAGN4FGL J0730.7-6602?ÚàtSŸÀ4ËݵR]À:(›)¼'ìÀ<Q7Âäì~@!>{ßI| ?û†×¥mã2?¸ûŽ^I·?§¯rÉÌf?ð$ύqm+@ó…'P¥¿ïäY`Äeö?ê$õî.Fd¿©7q@Ñƿޛ0þ$³"¿ÙXÜ¥‡äe¿Íóÿ*AGNbll3FGL J0730.5-6606PMN J0730-6602?ïàw* ?\ù_¸ò?<qUPXH?0ÌôAk	?kä]üKÑ?ZÙ>¢È¯?ïÙ*Ç1Šð?u}ƒxI?@`U<x<Ô?I€¢Þ§?q^'½ —-?s¯J÷CD®?ïlÂ^ðâg?{O#±7~r?a·\rþ—?XËÒÿÔO?52å·S?y½ÿ?›u?ïÃÓî˜é?sX/†sS·?lâÄ£1?PF±<L—Þ?šK3׉C?rl!¬o)š?ï¶5ðc,?s±òôXÀ?T5>ül.?H¾!o°¡Ò?׸!êÂs?qé¡2
Ô?ïk4×M.?‰ËŸÝԌ?TՐà¡a­?i&_m'e•?‰J€¤!ªA?‡µS:bó?îéMÕº¡?‰ôgï+?lÓu6þŽÐ?h™R¹@Áý?ŸD'	?ˆ¶4OªòŽ?íäÈêó‡?O¶MMs?|F¹ìV5?gk{Çt9ã?®6ì7a›D?Œªr'2AGN4FGL J0731.2-1403¿éÚþ>gwf@–ù%ñ+QÀ:*Ógñ€áÀ;ʎo™ëÏ@ûL¶çÞ @/<c]j?п$ÃÍÕ?׈'=Y@·kcü(Û?ø›{HË Ó?âñn!›±!¿éçÇßþù¿Ü$ýŠ·¿ÞŠ0]¿î1ВT*ú¿ïùžrAGNbcuPMN J0731-1402?Ó<B;
ó?ÂwOâìHé?«V¿~€o™?£ -Óêü¢?ä¬rêƒA?Ã[=E¹?ÑD`òß4?ÆùO6Éì?ÀÔÏ
+?³Á‰®D?ƒ?ã(›¿†	¼?Äãñó^I?ßõ 't°x?²k\'6ªµ?ž~%ó`?§;¿*Æ?Ö» Ƕ–?±Fs¿°ÓŸ?Õ*+ÑÑ*?¢q'~>?Å>>T#˜¶? ³€áÁð^?àdÕ1>?¤Ã'"ÜSO?Ä:üãv¨?¶n§´·P?­JeU¤Š)?§Üü¸ÖSg?éšqþ"?»nNDåö?·RpýM†?ºl?ƒÎ-?Ár^»»ò#?¼=_qŸ?è¹1žLv?Ââ5'1л?ÕC5•ŸJD?±ef•¯‹?È'¥ÐùF?°#-:ºÝ?Þ¼	x9?²‡½'˜Ç?Ài"ñõXæ?šFæ]×?ÈäÉ>‰
ì?¬Ԝp?å¬lsàfK?¬Òçÿ9MØMIXED4FGL J0731.8-3009?äuÙy¿šÆÀ–4T›bÇÀ:nb
·'À<'‰±Å@ n·Ã¦3@ʸ¥Î[B?ÃÝ
Ý~ Å?ÉÞ
¼×?Î*ÚÊ"Ý@åàÄüI¿å˪Þe{…¿ä¡L`«¼\¿Ø^ìŸ{¿èZa_ìNÈ¿Éŕ 
;¨¿è,¾|¨AGNbcu3FGL J0731.8-3010NVSS J073151-301058?í'~}'?§çëg:Îg?d"¯­Öµ'?S5°•Ñd?¶{6o¥?Å?§­4¢Œ?êì¡$8ª¨?¹^Mþ"7?W÷†'¶e?cmçB#¥ô?Äy€R(t?¹)Îõ4ä¨?í³wÕéDì?˜¢©áÛë?u[•8Ÿ r?h¿µ{%?±‡þ_Ô?—ŒÏÜ8Ž?ï:[±Š.Ë?sc¸P±ÐÊ?Hö©>!(½?3óf"á…`?—ìԋ$dM?sQÂì×Ö?ègºZ?¢¾?ºðKWgK?zi=—4?h‰jª›-?͐ÓN"ƒL?ºÃá"¼à?äìÆ´Ã#?ÅH³å—–W?\ރø&'?pšuÊxñ?Ö	"¶¢?Å>ޙö-;?ém‡Qâ?¬7ÆÁ+??‡õ×Ý÷íb?x‰™fVíÁ?Èʅ:Îc?«m¶/à?í¸e£.)?'&#Þµ
A?`G"@ÿą?SE,`'`?±º–Jäè"?'#-0ٟAGN4FGL J0731.9+2805¿ë:pÊ@4¦£ßm¹AÀ;3x‰|ìÀ<·v Í|@ M«¤?þ{Ê`áÂ?Ю†ü#»?¼'îY?ìH^sRÝó@`¨܅ý¿ÕIÈ`u¿ë!ªªcy¿×ÖRß¾¿Óòó¨é¿âÒ;66ó²¿ïÿä¼­šØAGNbllRGB J0731+280?ïÛ߁QƔ?r5òfu'
?@¾½Ì ?Bæ"Jã$?oðÏAŽn,?p'¥î_?ï G½Ñ(É?Ÿ"L2—?[4Zláib?`ê82?"‡…DøØn?~‡q—Õ›¿?ï{ŸI˔Ø?tžÞÈ7ê»?_žÒŤ­?ZöœÑÝü?$mpÁO?s®ÃFñ	?ïJ*R†W?lCU–'¯—?_ùí~w?A4q
Ø?"»ց¢?k »aîo"?ï±ØýT ‹?w	¨Yñ?MB°äæ7?Aʺ+ä3?µ•™Fòà?uґHA7?ï–Œ¸¤f?™7ÍWÔV?kÈmq¼i?wê¬WžŽ×?œlõ`d¥¹?–À	OG"?îýõeêŒô?"æ'¥©?g'¸S_¢Ï?aͼ·-	Ã?\\>´+?ƒÐzx	…Ÿ?í÷!hÊ2­?Š½hkm?pùsß?[àŸŠ<a?®}÷OøÓË?‰váAGN4FGL J0732.7-4638?·sr/]ÀÄÀ)«"«CIÀ9ù±ñ\ÏÀ;·×Ñã@"ñ>q)ä@Õí6´È?ğUÆ0%?ß±Þ¿"~M@9½ÆŸŒ"@oÆÚðQ?ÙÉÉã
€ò¿Þ—$'¯À¿çXàÚö±¿íÞ[€px¿ïûE@Pýô¿ðAGNbcu3FGL J0732.2-4638PKS 0731-465?ì§ÒE¬?¼$ÚaØ.¢?©Îù_ÃX1?±)ØònÊ?«³å?øM
?¯vùi_€s?ïŒ{‰5?¤C#Y««?'}W/VM?ŽE²´;™?•/í]¯ì>? Ewgnê?è`š:"(?°Q2ˆÏƒ?½dÉíê4?¦~Ó»@—Ò?¿–dgÕô‹?¦îMõÞc?í¤´Þ՟?‹"•ëÜ~é?Œ6?%Û?oÁC¥pæ;?®§1Lr,??‡o¤ñT"?ìÀ‡ÂÒV?µgQräN?§eZúV۟?«LÞ6ùÞ ?¬'3k3Í?¬ù6¡Í{¼?íO%/íâ?¹yà6)Õ?¡"6¨U?­Ã®‹±3?©ï¹sÅÎ?±¿­Í¢²?çBV¯Â®n?±];w'éN?Á1ŠÔ&TË?©­ùAݶx?ÁÅj©/þ?©')P
£?éLË_0ßh?¦øå^²ö‰?¤VÔ)æÂè?Žý¼¢ÀÜ?Å·x‹×å?¥&>ê1ȶAGN4FGL J0733.0+4915?琣ý(gÜ@:ÄÝ?á—_À;Ž"çƒ1xÀ<ÇÓØZ@ PÊwGà@¬Á¾¢h?ΐä>X€J?¦ƒÝ‰wQ?×ì$ÁUuR@ƒ,,®´´?ïÉ÷šÖ°{¿í',ˆG¿Ò–ñH­ü¿è]b
â¿×óµÄÈqs¿ß¤L%šAGNbcuTXS 0729+493?ïHŠR U­?ŸA¡­[º³?L4ž	ߣí?I þÜAgª?–
ÉKÄí?Ÿ%'+®å?ït"¶ÍK?ŽCṌœ?jOz7?p¢ÉgMÓ?Œ[K6ñq?ˆÃíMêX?ï,@M«?ƒ"œúã?`Ø`£‰ªŠ?J¹¡,ì{¼?˜\ê8Xç?ƒ2
Õfàp?ïŽrü'?pÿäͯ«Á?T]	Q'±ë??;#çð¥~?Â]òŸP?qCñ:x?î+[ï¶x?¦™/N?`!#tüçª?VQÙR m•?¬H.Ù6†ˆ?¥àÆ(Ï®?îÁ°¢s? ÓÐ̪¡?s¡yHև…?€8sñŠ¸?¡{E׶Æâ?ž‹e·/{?î3ØßwØ?–Á´Ñê?jƖeÔ8†?aFlom·Æ?«£9@î?•(O²ùE?îãæ¢i?"N؈õn?kìeƼ¾?a¯˜¢Í?¬Rû5Ò,?"•Î ñÙuAGN4FGL J0733.1+5910?æëª)xŽ @<KªX-¾À:¾åžTê=À<¼:ìe‰@£³1fª@Ûä—Å?‰Å!Ý ?½Ý¨<I²Q?ö-íy¾Ô?þ:|PªC?ï¹Ö…³2È¿à˜›¢ˆU¤¿á½Aԋ³¿å^ˆM@û¿è܄›Ó¤¿é ÷IíAGNbcu3FGL J0733.3+5904GB6 J0733+5909?ïZ¼mÈÊ#?…ãẐLM?n*0_Ù+m?aÖñЧ¡¿?ã,@Âì8?ƒ…–ªÛ?ï'ÂDf??ûà—¢!?€£ià$-?|…Û>\?'¶‰[Ù§?ƒ¨²—Ÿ6?ï,
Pw"?‡åŒd¼h?}¹2!|?~O¦ZÄ?"ijãßÊ?€A†Á{d?îš\6%š³?|½'Î¥'3?—ïŽøé¦Æ?stQM\úŒ?"ÄêGŠlÑ?q¿;y†´O?î-ÙÌ ¾?œg7eª¦H?Š`M䨠?~w
²J?¦–næÄmù?™qcbš?íì5yå?¥¢¾c+;?'íE–¡½a?–çzÿÎÍp?¨F
0Ž>ý?†
rDÆ?î<ŽIÀy"?•ŽÓ@Oœ?Œö÷Ùðëž?‡¯þÅÇL?¤ù]o3ùÞ?'9×PÚ?ì<§Bψi?"«Ì"ÏôO?®ä
oñ?2z5,/ÿ?­Q€ÆÑð?Œ­ ²s¢AGN4FGL J0733.4+5152¿ìW%%Q/@;PÜY1ÊÀ:œ˜¬3ÐÀ<'·I­Èü@ ëË|Àšå?üWu¸e?¾Ú¡ Ì~H?¤õg £#?éUM9n·@)Òh@Ž¿ë"Š.B¿á՚ }#¿ß½<:¨¿Ô;»P¿ã1Vº ù¿¾™AGNbcu3FGL J0733.5+5153NVSS J073326+515355?ïè²ö%Ðc?Wï_ÍÅZ?@?Y";?1;hîߋ?c="beß?U%'¢ˆ?ïÉÓ1¯"G?sÆÔñχ²?H¾^qŽÕ?Nªé÷é2?wþ£î4,?qˆ/UÚZ[?ï–îw#å?n*Ëæ‰ëˆ?XîL_D—?A1[Ó>Ÿ?‡&˜ºn
?lX1Åùâ˜?ïSbxΦt?pø&{Ü?c˜e3?G˜"Ú'ì+?"ýÝw%7?p°ÕA|€?ïÕç▧f?eZý_»I?Pác_ÞPp?Dõu$F?pӵ壵?a°ƒé͚B?ïk:\?Œb'ÉdæÉ?\NÃj¢?e6ç'ØëK?ÚSAGRb?ŠiÏÒe½õ?ï7'dŸoz?~n<‡9'?dÏyéeµÃ?T†='ûÏS?–sä4d¹þ?|$¾Ë:z?íö¸ÙzÛ?Ü¨á"Þ?z÷ÑL'9Å?fÀîdÓ?­5x>ÍgŸ?¤ˆsðâAGN4FGL J0733.5-5445¿îz¦Ç!±À0-VJQ]À9àª_ºz»À<M‹^¿@ô¢""EB@?A^o!?·ÐK\tË?±š}Å'¼Ý?ø–ùáØ͌@j¼¨'Zá?ïûbví'¿ãŒdý°šg¿âdøbQÙ¼¿â/! 8B¿ãɵÁŒä¿ì"~w=AGNbcuSUMSS J073334-544544?ïø&øgZW?8™ÈÌ4?!#êsrÍ?ú¶¬Îpb?K#¹¡¶K?5èAM•]?ïíœhUÿ¼?h|®Fb܌?.	ÜvI2?<'xP¾E`?`'ù÷·F?fƒ‹Ò:Î?ï¶[p,ý~?p2؀›W?]Õ2øÖæ?g/Ջ-_P?}\ûD¸£k?c{–/t[?ïáüN<…?NŒÈÈ\Š­?;Hk#1õ=?¬ý.?jš¤VmT?M€Û–ç`?ïõhÛ>];?Aߌõ–ò¥?."0§Öx? ¾ub1Ê?Q]ÃD*ÙË?>å<.ÿ?ïțØ8:Ú?'"%Tž?Eâ#á%Ö?[» Úm'»?yˆ§jÓ?H)u«d?Œ`‡;?|#l\#?j\/©W|?qÙU'÷Ȉ?‡|Ñö®H?u¼Í`{'?墳ó.û?l£+ºØ&r?S—'lD4'?>žMÿhP?ƒ'Ö'Ž…?k^ul˜Î{AGN4FGL J0733.6+3649?ïñ‡—©@7ѾãÕýÎÀ:·óáäŒÀ<'³!*3@x\fˆJ<@°Ò€jôk?ÂÇ·#Ã(´?¨÷ð€ÊÚs?ã:¿ïn¸@
<åc?ï´èâÄ0¿ç+zl­¨D¿áֈ7q†U¿äx#'¬?¿íë¥jˆ4?ÑUÛ}¿žAGNbcuGB6 J0733+3650?ï݆%s'?g¤²˜‹?FSõé5?;ãÛT´"É?löE¤trÿ?ež>Qj?ïÕø[,1È?r1ë/€‰?G7åmÒi†?TõÈùR?rÕÙÿÐÜ?l«s½!?ïvh£=Ã?ƒü¢ÚC"?qleèu ?|Ò_üD¦?†ìdEvc?|òL¸~?ïÙ,‹Æ"œ?OíÉЭ" ?SÆ¡5¬?6¢$y¸ã?lðfµ¹±L?Jë£{¦_?ï¬Ó¿°/?~õº¸gØ?ZÇ"g(Æ,?R".·?¦¦Í}¯€?}H7n,·?ïŽÔÞWþ^?‰ãsŸc?Vn*Ԍ®(?bm·÷žè?‰}¨€ï?‡[Û¬ÿq?ïWkæqÓ?*Òì•wÈ?zâ%åoîi?ïµ³jK?–\‰
-¿ý?‡6É®ý\?ï‡ßa=ÌX?p‹"AK4i?l…ÚUd¡?V L²|fÈ?†æ±¼C¸?lâ,3AGN4FGL J0733.7+0205c¿äýÎnQ[+@$º±NÂóÀ:¬i—sN¬À<"/|@5@Í$¶n@è"C ç?ÑúeŒKÓ=?ϗ
Éĕ?÷›bÇuu@š1P/p?ޜJØw{?ïڍ¯ãˆ¿éÔ¿?E-¿äÙÇQbÉ#¿ëä¥Ï2¿ïÿú¡œGtAGNbcu4C +02.20 ?ìæÆk+?¶16Em?šS‡I\€º?"'€žìØ?¹Sçý†|?´–Z‰÷*½?íß/⊓?±¹-òd‰?‰#]»ª	?Íô`Üá?«Ä*dH"/?¯Î)Dý?ì¦ÓÒ-<'?¢C©ŠîÕ?™8ùƒª"?$aký?‹?´{#aœ¯?€Ôv›Z?í‡Ð4úøH?Š^Xi½LÁ?—¸ÊåZ?yR»¸ò?«¦—ª'Kƒ?"°ÛËû??çd'ˆÑ?Áçv©!v?²—½˜[¾Þ?«‹Pe$?É!ÛƒâÅ?¿œÄq^'?êÈé9®¼/?Ã<Ë
]"ž?¢bõÄlõÚ?¬©JÍÓ?ÀC¨`ˌ?Àö»iù?èw]ºÎÑ?°œø¶ø?±c&ÙÍU? Á¤†6Ú?ÅqWÕ?©zçøËÖ?ê>ïî ?Í?¡Ö SI¸?¨°™hÕ?'nc¤®åJ?ÀØw¾?*b$€XAGN4FGL J0733.7+4110¿Çù2ÆѶ@9
»ìª¸¦À:=~|Ý¡0À<yy1DEª@i%u°[R?þÙ.T§!B?ÀêÄ.˜™¿?ª€câAm?î]eÖômü@ݤ]ÂÓпØC¯AÌ~¿å5f͔s¿áˌ%<Ðk¿Ö®êäâ¿ØãP÷,r¿éUÂ@þAGNbll3FGL J0733.8+4108GB6 J0733+4111?ïÓ`þÑ	?qåaì ¦û?QÅ¿š8À±?G*ìÁ²Ÿ?r_||§??oi2³Û^?ïÏ}q¥y?qñ­2!î?Ká[ëª~?RbªÞŽ·?tßX0ëʲ?m÷µÔê?Iï…?r•°oôƒ?a:nwÂ-?K~…d)'?ŠòÊLØR?qh©³¬?ïcÔµ¤g?fŠŽh'?iê­*µå?G€ÂÛǵ?a¯Ï9YU?dâ©>|?ï§oíÆ?ue$ö›.š?aƚ$AS?Q,²{íÖ?²^'ô?rçPÃÔ6?ïjÏïÁïN?‰é2D\«?`¶ìã.V?i%ÞLV8Õ?$bÅMü?‡b'l†…?ï>ît´ª?ƒÅŠMø6­?j¹¯.!k?Z¥Íçz—?š@þü3'‹?'®^†ÍÖä?îdè¬6?ƒíœÎFèN?Á¯6`?e=¨QJO?¥Ð}x`ñ?'Ãü8\'GAGN4FGL J0733.8+0455?îÍh•."­@']—5;À9ÆØôù;ÁÀ<6	'_Á1@O}–®®@ÊZ¤'Da?º8vÿeÑ@?¾V§V›˜!@€ê[Sí@š˜jÅp¸?Å8(%
*¶¿å(Tf,Û¿äP‰OŸz"¿ä`
+Òì¡¿î`~oò¿ïÿâ~9ì¶AGNfsrqGB6 J0733+0456?ï͐')ªì?o³\øwJ7?Q	 ÒBäs?F}¬¹¤Ù?tõOSvˆì?mk¦›¥'o?ïÛT†Xãá?vó¡Zª±Ê?B‹Í
å¿?Qaøl/¢‰?pY©Þ?t¼ñÆ?ïƒDZ¢ä?ƒn›'Þø;?tñ·0æú6?{R]
\?"ÂDÝ(?z©8;dhã?ïí	'"~?B+ýuË4?Býš˜¤†L?'ÛM²ŽºT?\oS
&°??$xpW=˜?律\£Ž?÷wôïÝÉ?g©0ã')?fm¨xÿK?€/œ¾zÄ(?}Ã
'ÿ?ï
n\ÿ?'ð¹Á T?XcAƒ"?r	,5}dT?…»A5ߝÐ?al49K?ï5*«i¯?Š;Áµ,q?€? m`
+?¯A'¼Ë¹?':ÚUþ7Ÿ?'OÇ8oOr?ïÏóã5´?`"óÚ>c?Xw¬GèÀ'?EJEȌ?r:û»
?\rAŒw}&AGN4FGL J0734.0+5021¿ÕÙÒç¬@;$"ƒ‡ß]À9áj'"À<gœâ#v'@ðy©åE@&ÜB‹•Ë?·ëp&É?Ä¥"¹¾R@5\FR@Àx¿¯Wò?ïÑ>¶ôô3¿×þT.U}á¿ç6òl¬Ò¿çÆžEÑ¿èX.•>Á¿ãò,"à`AGNfsrq3FGL J0733.8+5021TXS 0730+504?ïæ˜üÌÕí?^5†œ×.­?Nî€©Æ&?DÓ.¢¸Cü?aÇÍhüâ?W¹l€+ht?ïל]ÌÂ?pêÛÂ\?M@§Ÿ©Ñ?WhŸÉ¯ò?pÐÛ~{'?jKÔU1?ï õó%•Ö?{ï•î?iâjÇuÆ?rH¡ú
?IèªA"8?rUð4vxY?ïÊQŸëÿ?TlÕÇÄc•?g/*"ŸÌ¸?Fȧîã?nσ͵Ä?N"Ï`¥–À?ïЙÆCj?fýýš•°?`ì;7››$?VL̆àÀ.?nyþ¹ úú?aZ('7¢¹?ï~ù´·W?ˆj-Í€?bGP§|ù?i-cŸ9|?‹í-eIøö?…úÛVg?ïYíwYo?ƒþæ[Þ\ö?uýU›‡ïD?uýµ1)Š"?Ž…÷dö°¾?€—_«'àÁ?ïSenÞsØ?w¯›ŽéHÎ?'å1ÏY9Å?hMn¦ƒ!?ˆArm.K?p«_©°«kAGN4FGL J0734.4-7711?ïØ\³À8
à"S.À9i)•ûhÀ;ç$¿ÒéG@=@ޗz†@nXæK#?²§òø°€f?¾³k§ÃÓÕ@
í$%y6M@žL[Î2¿áÓ_
+¸¿ßM"ÜIm¿ã¤;é»¿ä ˜%ü¿éã{dû,\¿ïïÏ0T[¢AGNbcu3FGL J0734.3-7709PKS 0736-770?ïó2£ÚÿÚ?L1¹"žÈi?4>{ÂrÓ?,•"ûFv~?T‹v0ž?HN–\??ïê»u6Ü?gvv'x$?3
‡~Ä>#?@Wƒ%¶?bâÚud?eö1'L³?ï­û
Qø?vúúªÿ=?chç§Cþ>?k\²R4?N"Á˳?q‹±G?ïâ™ÆB͎?Kh8ðf?9''4j8g? ý'q¸ˆš?j4Š*q?I§O–É=ÿ?ïçɈ¨8K?Y矄gÊ¿?I1—O¤'?E'‰tÞÅ?aêb=ò?T]v÷¯Ùµ?ïÄÀӉ\?€Ÿ°3ð?M½J6і•?a*Ҙ¿=?yçí»?}Öª¤9¡?ï{øhèÂ?€ÐàS¤":?m©f/Ò³?oŒ~Æ£?‰—Œu°
"?|7"?ï»ø\P@"?gIûÒkï?Muñ;þMø?:G3¨œÁ?~U§Ú~?eâÑ@+î‹AGN4FGL J0737.3-8247?ïIqD¥–À9y¥CñÇXÀ9ڛ<1·À<8¸¤ Ü@ýäG'»¯?þ=þÈs¢?¶_l÷úøÚ?°ö!YìÛ`?ûz4ääÇ@9CiŒ5®¿ï£Ùqö½?ïÿxPsµÚ¿àý|Bם¿ÜS¿ð›^¿ÝĶv$J¿â°ÚÉÒ+AGNbcu3FGL J0737.8-8245SUMSS J073706-824836?ïæhàû>6?XËí켈??Èމ4s?2öGœ…?ežmÁ!:?U廦ÌÂm?ï´§Äw
E?xŸJ¤?Y]*ÆÍz?b‡¾ØôË?TÒõmÆP?|ÌB¥¢T"?ïQ²øeVò?qAåiX	?pmŽ
à§Í?p֌|Hh?'®=oÁÓ?~PŸÀV?îÐÁg؛&?v LÄZ^°?""ì™!ä?d˜ö7%šg?›Öq/OöN?r¡op1?ïÁ²î»p??ps?¿üI?^þCYGw>?WX	™?wf÷èÒºi?jÎÀP[f?ïÀÕó'	?— ôfJµü?p‡(ÆMLÔ?xúԟ
'?˜F]"±?")ç³l¤O?î¶`›±?é$`I¦?€VTÔM^ª?7<å‰E? "a–/Å?‰Tb)2ä?íƒ"|V½§?RƒÃ_ü?"ž`ØÑˌ?~'èÓ£?­~§Ë—ŠÏ?‹p§•­<>AGN4FGL J0738.1+1742?暣<ä›@2÷ß (À7@'§À:ÿ³"ý*c@[‡/‰°m?ÿ¬BÊ ?˜wñ†É?®îŸ&÷@Ý­àx{<@Õ r'B?É	¤C–­¬¿Ô<rwá¿á;ã:Í[h¿ßJål[¿âÔOb"Èõ¿ãY™~Á¦ÿAGNbll3FGL J0738.1+1741PKS 0735+17?ïâOB)è~?fFºééDÕ?RZ´ŽÀŠ?O6W?¿ˆ¨?dƒ¶?Wé?c%cÌ4á?*æS?Œ.Î8éž?kÙɏ?s–ç¿0?‰T¤³?ˆ0©½"zÀ?îU'6OÉ? ýòÒ£"?I;¤Æg?‰SiRŒ¼R?¦U³ÙÍ?ŸH­\ý¯?îbŸÌ°ê?…VLr1fN?€å9•vîû?cZÏþ?¥œ´Ëâ¿?ƒPûBÈ{Ö?ïØ5Š•3?iPmö?Ps÷(U®?IðñI¬—»?oyÆ#À?fˆ Š"5?î"ÁȄ5&?¦ÙP!';?ÓD7øÌÓ?ˆWéÂ0O?¢Ol&4k?¤Ó¯ÿ…³?íí5bø?¥OÍÙÎ?¦fÛ{D?Š"VY7…§?¬Ã){ ÷?¤°<J†?ìŠçʪÑ?œäÒy Z?'nžšêq?zo4U}H?·M6ž?›UûۑUAGN4FGL J0738.4+1539¿íê2X—Ʊ@1O\žf‡ôÀ;mÄ@6PõÀ<½Üºí§@ °€¡¦‰?øT¨Ù ˜?Ø̙¡&V?âØ\î 0@t¤Ú¦@UîcöIž¿ïÄà\+¥?ٙiþX5?îŒÖ!à$˜¿Ò×ɓ\i¿æŽÏŒ0û¿ÖÃT¦Ë±AGNbcuNVSS J073824+153839?ïÄü¶\Ñ?lëM7¡›?aFîa'#d?Us¬V~÷‹?túªpÎi›?e홧*®¯?ïT…%ÌËÔ?"눂M«7?tM t·­?|y˜&ºÅ\?\$•£¥?ŽkœV'±?ïÍ9_ê?Ž€&?ª›è?wöra–"å?zŠ6W.å?˜ˆÁ—$?‹%avX?íû\ÛUÚ0?Œåb:ŸÈ?~aqò"'5?g—IEãË×?¬~%ª?‹8û"3?ïˆa´Œo?~$ý>Eg>?tü|þ±]õ?k6œfØó?ƒiTiN!E?v©½Pr|&?îTÅi"¥¿?¨å=ÃO?ˆQo9?–ŸEzêt+?¤²(•§E?¢]ˆRt?îM.p?š²µ-ü?€«âÄøAl?i]Ü45?§Df¸ûò?—ã¦9W#?뱃0T9F?¤^ã7&Æ?'óÅú¢ô?x€î->Ú`?À
¶ßy?¤0X.â÷AGN4FGL J0739.2+0137¿ïE	Õ6º@&Á,I4&xÀ7')yv
£À;tcŠ	@¡œvmŀ@'>3Av?"[M¿·¡©?¸T=ë.H@ "¥Ξ@Wˆ"MÞ¿ÏòUk`K¿â³¼ÅîŒ:¿æL¢:Rf¿æ‰Ã}˜²¿ëÌ>1"÷¿æüÇ0«™vAGNfsrq3FGL J0739.4+0137PKS 0736+01?ïE͑îªm?‹•Í·Lj¹?k^»ÿ?e	†ôÜ?"ÚvVê	®?ˆØÑêxAK?ïŽû}J?"®†€,?`È5ˆØ?lFêV"Ç?ˆ@ø¢ü_[?'¸OsM&?ï>}éÿ|?'x»Õ82?"âÊÀz{?‰Ž£Õho?‹—Ѿ/Bf?ˆ¶i 9>?ïñÅö¢g?Gݓœ£¢‹?=¯§úI]*?1ë
•§<?VTŠv ô?BÂJ@?ï"Ö"õì?"–k'S-¯?m`©î8rÜ?fº	‡¼q?™#O÷uS$?"tÙ§Ã×D?îêg9Êüé?­ÿyœd?q>"qåí?ƒ¹sw¬É?žc?  i?¬þkXÓ%¸?îӌ˜ex;?˜‡ž/ۃØ?;-hóþM?'^ýÐö‰&?•S?ˆ¥,T?'‹9[J¼?ïÚUQý4?c†'Šj`?Qô:Ä[Á?IƒDÇE?l°'2bíÒ?_kQk…D°AGN4FGL J0739.7+1743?ãÃ×ìÌ®@2qWÿ›V2À:˜)W_À;mÓÐÍŽ@å4`t	@ôZDïô?ÊÀDÔt?²ëJç.ù?ï+üÞ@âaFkõ¿Û0³¼…à¿éË4çhY†¿éôàM/¿Ý´áÙú2¿èìЮÝ*¿ïùÏdVÁ®AGNbcuNVSS J073948+174304?ï3¼F±"?«@Hï'æA?d²Ã*œi¸?z	°©½À?–òÄOön?¨ÏBLF?ïšþµ
y¡?†QPþª}?c™_òÖë?nnV6ýÉî?"YúêŽÌ?VGµKQ?ìå5C%;?¤q=/æk'?ÛÍ—á?Ÿ—bò8x?´ÚÜDŽû0?¢5oâ0Ï:?í¾L%l	?ŒÅl¸
m¿?q~õhU?SŒÐˆ-?°õ¯'l´è?‹õÝÌ«=&?í묡ç¤r?§æ¹He¾Y?w%r_«Ò¥?|›µs®ê4?®`‡'ü‰?¦l^åøôœ?ïFWÁ÷ ?™–r.l?s¤
˜(»?¦42eƗ?˜®2[[–5?"Í9Ÿ­¼?ê	摈Ã?®'9'EC? ú­*/ø?—™Ø6PØ?Ý"]Dv?«ð-5`?éŒÉfˆA¥?¦~C»ŒJ¶?Š©~
"Oû?sn Âät?È"B""Ó®?¦'ÝýFžAGN4FGL J0739.8-6722¿î!܋ܗ›À4nÑáÃôÀ:døÄ¢[àÀ<[~ùc@ñØSŸ@ޝ"ÐÜý?µx…ø§ñ÷¿µ€°®ˆ"?ÿÜazn['@_"ØaV¿äw6b'œO¿åHþaur¿â÷<b|¿ã9wÑ¿ßØB·4µ¿áWß_¡{:AGNbcu1RXS J073928.1-672147?ïé™Q¨Ç½?y¯9µI ¢?0Ä«³ÜÊ{?-þVøw}5?dNÈiõ?yY'£ÏP&?ïá@ìF?j—ªoïjö?8!7¶†¿?F»Z¡?k»Å_8~Z?g-XÁ-?ïlþå	ã?±ºõV{?Rý'r"3?XJ´Û»Æ?'0JEƒF?'Oá/S?ïÆoxçP?Y溬?AµVßß4?'¶ 
<¥?z§¬ä}®?X²ê£rî?ïÐ^¼Ø^?{xˆf9D˜?I6Sõ?GÑx‡íöñ?t˜^8Îe?ydðcÒþ?ï¦ò,O5À?Ú¥3ê¡?L)ah¸- ?bŒ@Œ­bý?"€ÞÈÞç¾?Œ$Íböy¬?îÿ7©B6º?"jeͯãÂ?_ÛŽ
Ú?`Sî6eØ?ž(ý" «ì?"Q-¬üñÚ?ï4•¹1?~šß#Åb?^N…r½Ü?M«ƒe@Ñ?—ˆw"Ý$'?~Y€ç&ƒAGN4FGL J0740.0-0753?êNÏ¿Ý@EàqÅ?:À:†_-À<ê°¢¦@µÏ‰?¯B@µj£	#?Ĕˆ7Çl'?¥ìã¼à?ß¿½WÓ|@P`ö:¿á
B[Ûs¿Ýbyýr-¿é±	ÝÏS¿é"ÛÈ¿í;'ô:Ïà?ã0} g(®AGNbcuPMN J0739-0747?íöÚ#;]=?¦ó%M­·þ?tÂ\>@î¸?nÙ̧õe:?­úF§ÏÕ?¦4´@"ª±?í{8 Z}û?³!3Jgÿ¯?nñÍQÊÕ?} Ð7kù7?³1»n=Ó?²)í$L?îZ bԔ?"'Þ_3{´?~\*^ág?v†yñþs…?¦'t'Ѩ?'¡Û·•:â?ï«8ùNi?d5"'>?VZá¾…9?=¨]Ð$?'mŸµþWF?bJâEQ?ëD!_´õ?µ¼F"O]?"Þ¯?¡•6?'þ%!/1?Á¡¸K?´sßår$?éÙ+,ó ?ÅY®"£Õ?|¹Íþ½k?‹½uI‹ÂÊ?ǵ…Œ¶ '?Äӄj¶?ëȆšA÷?¤ºžë`?'ˆÎsª—z?"Â/óŠ<4?½Y—Âïî?¡íPüÒ?îìòÀŠ~?…©Åö>Â?qIµïþ7£?^1àdž^û?ž:kÇàe?ƒeÉØۉ¸AGN4FGL J0740.4+7300¿èm*2X—Ç@=l" ٔ[À:¼³ÑSDKÀ<;&Ö-Ÿ@}EÐïœ@
«£|qk?"f7.¢¿Å±KgŸV@øpž2@×´³Pz¿³·†
¢¿í^ܙÉjB¿éͽ"¨™¿À'Á¦Ss¿ìû2Ál"¿ïÿí@_Á‡AGNbcuNVSS J074111+725822?îÁÎ
Ö%?À²+¬N"?…‰àÂa´²?ªµ_}&?LL÷?ºT¬wKÀ?ԀÃ?"§ÀÂ9?rï?ªÆ*Ý?‡Š¡µñÙ?€[Ü4ÌÍè?'ðòM'=…?î&'fcP?Ÿ:/Ñ©ÖS?'9ºØvÙ?‰‰N—XE?©˜n'NC?ž	^Wâ»?ïØÜÕÙeâ?gzÕîj<?cD5¾m®m?`ّË;é?cÞôƒ©O?YÆþÈm¥Ÿ?îg ê!N?¹$ºBUe?"lý'Š<í?§Õ•ÒmÐ?Ÿžå èŸ:?±rT²ðø?î°óˆ«é0?¯ãS‰Ôz?uJ]ZôÏ?¦ªvQ9/V?š&鴗? 6áß½?í:æ:ºš?¤Î<)ûØ?'@­3°<?†B;ü¿à?³ã{-%…©?¤'þú+»?î‹?"'äª?®†g¼ŒÌ?¡áÍ&CH›?®Í#´»?…¨êPˆ‡?'Sj='AGN4FGL J0740.9+3203?磴¶¼¦@7Ϋ%(®À:®Ð!#~À<}æðdŠ@;Gxåo@¡ Ï?À<Ndçá¿ ž=ŠØ"?Þ®@dô÷8?÷úÚl1¿ªMìœöÆE¿å77¤±ü¿çÄóºw_³¿ØÒB­)¿ê0Bhv¿ìqýs]ÆAGNbllLEDA 1979979?ïœ4w'?',(	ÛâD?dǓ¡¸Äÿ?Yºø¹ž?ƒÀý<Rø?€a›–(?ï~°{¢& ?…¿\õð?mÜyBUä?mælµ?ˆÜÂØ¿?ú‡ªŠ«á?ï_EI"?‰É¿d"?zŸ¹g|?`cö%1ý?"öÍ>q0Ã?'œa+ˆSÕ?ïag'Ð?w¦ûgÎö?ˆA±F?kGIéΨT?"EȅA'?pZ*ý"þ?ïr|ì‡?"×£BúK?~`ð®Dö¦?tç~~á–?—™t;ÙMx?'›õ9?î|'ƒG??¢OŽR{"m?…;rRõô£?'ê'jS?¢ðÚ?žrê?š"ÜÂúk?î6hìAv?™GÀÑwE?'‰YEñ›?ÀÈe<£R?¤X,Ži¿Ö?'ºxüÂ?í<'ØÒa?"ÀŸá¿õ?¢VfÊ&Ž¼?ŠQ½ð‡˜?©à{©H?ŠÜžþ'ªƒAGN4FGL J0741.0+3226?Ùðoõíhµ@7òu¸eÀ;̉>؂ãÀ<çH㞠@#/p-ºxa?õ1©u¯¯†?ÙVùvy!?ÔÅ:çÝt?üGZ·ÜzÀ@œ0K¿ï÷û^ۂ?î3;5t¬¿ïÿÿ^ðP`?ïÿþó…õ¿ÔŸÕÖÀ¿ÛÒ݈óAGNbllNVSS J074054+322600?ïŒ#9ú‰?†µº²O`?Y±? {ô?Qc;«ÿ?‰×%V«Ò9?†Dvsò
?ïÁOIOr?‰ÅÕj]Êi?O:n'!6?`ùM›Ø¥Ö?{q
lxÆà?‡GEÎf6?î·Ó–ó?"üQ¿Q?kwƒÛ~E?qEúƒ9ì?¢ËVÕ¶í?"V‹ÿ‡r?íÏ.…?{ùì}‡¹?ZRO]#?T©é:œ)?‹Íº ‰Ô©?ysš$¬Í?ï†æÿÜwB?ƒ{'O7"?b}Ž›ð©#?]t:—s)?‰¦ÜhÅ=?²2mÂ?ïT'•Áb?šVhõë\¸?d-$!Y®R?y–M}Äù?'èǼÆ?˜=?lº?î!§}\ø?šU`‹"MÅ?nk¦=#?páÆl«
ð?¬K&àb­?™èRHÔ—?îƒ@Ýsk»?œÖ0g<¯?vPÇ9ƒ8??ïy‹	q?¤øH:	ç?™§(z&õ~AGN4FGL J0741.2-5140?쬋›¡~À+Ÿ™€o&)À:oèuŸ¿NÀ;âŒÅuÀv@\ZôÃ6@™çZÌË?ÎÐè:fƒB?ȶUýb–Î?÷—'Ôà˜@±»ÚN¾?à;ÅþÒX}¿ÌÛybí`¿æàÍûü¿ëȬ¬›ÔÝ¿ïÿ$=Çâ?ïû…|¬#	AGNbcuPMN J0740-5137?ï¤ûkŠ?×'
L´·?kÜðøÐ]?rH"}ÜàÒ?þ͟®?{"÷€d?ï>Yú>ÂU?œSFV¯â?z'™:7?…¨i!Hþ`?'Ze-)¥?–é~G$…?í¾CA?²À?›iƒb†Ä?‡€-?†¨\wqô?¬9ëâ{Z ?—*jo‡Ô?îoÃê¥û¨?…aÃz¤È?î$@À$I?fV€ž*·á?¤ˆ8FŽñ?'£oF
¯?îè>Û²ï?«†3¾Ñë?…dÃlbz?'>¦5‹¶ƒ?˜J֖cÔó?™Vå…y}Ð?íÜ̚Þú2?¶ÍÕ¾ìm?"žá(º¹n?¢3Y!C?¨cźCd,?²Úe"pM?ë(ආà?§'Š
œ?¡îèËBúu?"ó`B1"'?½Á…ääyD?£‹=îšþ?ê¶dñFSÌ?£–ŠsÕÈ?›Í5—*mV?ˆe2'Ó*J?Á¬Åˆc$?¡jD>ä»XAGN4FGL J0741.4-4709¿ëü–r·q`À'zŒûüÀ:
O"'ÉœÀ;üýòÆ@	ýå¶@©EÄ/oY?Àw€bæÕ?¼íÜ
n?ø©¡Ñv@
Q©BO†?ëö@äv¸¿åð×~+©ý¿èF¬â¡ N¿ëä3¡<]¿é¾Îqèz¨?Ú/‰E
¦1AGNfsrqPMN J0741-4709?ïÜ£?=`;?e)C@'ª—??ÈÓQ0Ò?2QþNËÒ=?oc¦}¸©‰?cæ÷(< t?ï\N&…œ?•z\åQy?bŒ	6Ø'Î?jº»œ¶ø?'$ºàâ~?"î¹£Ó˜ê?ïMÙf/¬?ˆ#/À"u?g¸C¯«t{?i•'7ò‡?"hÜ`´7å?‡EÌ+Öâ>?ïNIáÂʍ?pôº"B!?hÅ{»ˆdè?IÐnð1+ ?"U1Â?où"álo'?ï¯ÑɃ8§?}±`Æ ƒ¬?N>$2ÙÉ?EßÚSêÏ??''«fßÖ¿?|j%išC%?îNI–™Vu?¯>ÇvW½Z?vôªá9q3?‡\ðÖHIæ?¨<Ñ<)"?¬yrùðç÷?zé«*?•'3üÃW?yËÜ"²\á?yÕCSÈ?£\ÉsjË?"QUi0I?í…dþÝ@7?'H!ãǾ…?…áG
ß	Ä?pk…RÆf£?±¯'º?ÐXÂiYAGN4FGL J0742.1+4902?ï`Ê¿›$Î@<0_¿ƒ8.À;7—Œy À<º%œq»@©†f‹û ?þ¼‡Tów\?Øj×DÁ?Øoâ+XÉ?ÿQßá|‡:@åµ{øI?æZà‹Ær@¿çÞÖÜH¿Ç&£"o8¿æóá^TI-¿ïûü€¿¿ïÿÅþ&ŒAGNfsrqGB6 J0742+4900?ïH萛?®9ˆ^t.Å?|d}Ró	?•©Y*=Á,?Ã©Ä|I¼?¥ÉŠ³XϨ?ïÞ…´q?"û™1ør-?i<Ÿ'
?o'½ØjF9?†9RÊÙ%?~ÒâS²Z·?î£R¦k?"ô*Ä*»
?Ý'6‹?ˆ7ͱ*-F?œ­l¢O&­?Žn™¨ÂˆO?ï	"u5%?y¡zºŒ}"??OwT?d>{G•\?–ý˜#@V?uJ˓,f<?ï`쇆?–ì'j"¡?*uþ–"É?€ù³Yçš?•Q¶^©â?'4˜·<.ê?îÈ1ªût^?ž$pÍ=M?}|­÷³Îú?…-R¨×?¼?ŸšŸ&l‡?–ýÚÎҒ]?íÃÒ\Ñ	?œä]Wáøµ?'Dñ
Ù8i?‹%x9Áz†?ª¬jNúÐE?™ÀªX—y?íÁ	½û?•®GRYQ?…^NÒ¼t?yLÀˆÕÖÔ?®—ÚyIH?"­ð=À)üAGN4FGL J0742.6+5443?îykòu™@=øe×Ë.À8tÇåÝ?À;òc`øh\@š{ú!n»@Ê=p£×
?Šˆ¦úw¢?µª@8M@iæ@;Yr@üþËÍsf¿Ã§Íyps¿á¶vÛ)¿åÔþõhø¿ä_bцoñ¿éE¸põ6¿èŸ^ÕxlùAGNfsrq3FGL J0742.6+5444GB6 J0742+5444?ïåvÓW;·?[.€òø¤?S|LÍP9Û?FÛ,GàC"?`ËSú#­?U‰²T©5%?ïÕ=
fO.?w±ð)Rœ¡?HCÿ2âŒ?Y7ó—Röª?rXû·s8?u¼˜ƒ)Þ?ïÄÈÝ\š"?zŽžh‰I÷?`œ—Rÿð¨?oX¾ä&´?uME—´ž?t	±ÆíRê?ïþ2É3˜¼?ð¥IŸŸ'?	ðxë‡íŠ>üÅ6›©­.?&WMé¹!M?eÙ	.?ï̹5Z¿?qØÆ¢ˆ¢ô?Sü†PJ?J)0©0!?t¤CÅeµ?p—î½­?ïŸ#‡Õ³?‰ºÈtj¹q?ZSŠ'|Ü*?m©°y@Cù?"쬬"õ¥?†þœC;?Ñ?ï¬Fc«dâ?~ùW•vGþ?_ëšg|À`?g—‡c"¥?€ðóÁW÷?|µÃeÏ?ïûÌèâ"D?3Gž£™'"?Í´d˜æê?$®+SÔ?:%Lö·ÿÇ?0vZ¸änVAGN4FGL J0742.9-5242?¤ÒoùuÀ,,©¬6TÀ:ê&yçMÀ;Ó·?œÎ@ÙqÍͨÀ@yÏ.´H?Åkøa%3ì?ӉU^?±@=X «Ó@òÿf}¿ï¯šAµ,?ï֘ȹAÖ¿ë+:¯(w¿ç±_ÞâÎí¿êzÇw"?׆·¿ŸgºAGNbcuPMN J0742-5241?ïá|€?f®?gØëÌß]?aê²ôÞ©?`y|LDX?Y1™ò,GO?VÆPó¢(?ïˆÍå.K ?"õÆÅ
ö?t5(Ñþ?‹•dóz?ƒ±òÁ×
?ˆbá'$Üä?ìä|ßi?¢R}/¾z?™ýFîû£?"½ß!¢·Ü?²`2epË?ŸËl®¸?îäk ž+á?~ÈÈ÷LG—?‡BS¾lW"?n‡|±b€V?—ÑbmR2?vùØz~A?﬚3-»
?ƒô}¯œÿï?µÛ̲\?üHè]–C?cû¦íP¹?by·ãníN?îdÓù*½ˆ?®Ô(ÖuÞx?'¨YúÁ? Òã3¸á€? ^ÄÆ ?¤fòl2r?ëÊq³C?¥ó‹ÆS?£öŒLŸ­ê?˜ØGœz3?·³öL"_?¡½™ƒ=D?ë÷³«Ç!E? wå%{7?¨gQ½ŸÎ¶?"«Z#q{?´¹Ä®Ü|?—i|Q|wßAGN4FGL J0743.0-5622?ÍÿÂ度ÒÀ/G™€o&)À:@NK½m´À<&¯söqâ@p|ЋU@w@GD?Äym>Ç»ì?Ãô¾""¥?úmlP‹3@"¿ÍŠâÈ?ïÍa¢‡Sò¿æ<|óp¥…¿ëDžj䥿åzÁҝÇ&¿çz4y"P¿ïÿþ½à ¿AGNfsrq3FGL J0742.6-5623PMN J0743-5619?ïô&ƒ€R?Iý¶HJæ?<'Z•éðˆ?3‹؂…s?P©"ÌÔF£?Cr^qÞã?ï×rP2%?t\Ò8{'f?G\Ãü¡Ø)?Q¸ýŒY&y?q[?dñ{–?rrô4¶é%?ïr©
ƒo?";Æè¾i?kÔÊpÉ»#?qiT?;´?Œ‰ã$D[c?€é`_õáª?ï°±-ä?[õ¢wš['?aPŽ+0?AÛsò«¯¢?%Ò4†=ž?X°'ÅEî?ïêé:k¶²?Y€ÕɼÊ;?K¦–½ÐM?Fï¯împ?\Z@\ù?›?S®'5Ú?Uá¯?Žô;îÇ6?`ÓP–豧?qkjÙª?‰f–R‹ià?‹ŒnÐҜÄ?ïàËÃs™?'êÛa­G‹?xr«òYt?zX†‰†xî?™g;†:'?/c¬b?ﶈ×?|8¿d.}Â?|´@ÂÈ|?c͟Òæ?˜pL9·?xÀFÁÚOGAGN4FGL J0743.1+1713¿Ç;$™<|ˆ@2÷4Ö¡aåÀ:tt "ôÀ<UXª¼Í@îˆv܀@öQo^?À4X6ÍÇt?2¹ˆà?Ò
þ Vâ@"µW¿ìa>‰R¥?î'úC'œý¿ä£< oK½¿à}á,U¿Þ»ÎÍ®¿åëÐ}ÜNËAGNbllTXS 0740+173?ïÎ2ϤÝ3?`¯hBF'?U¥"éD5ê?B?÷4Þł?s}6ñà€Ô?\Ç»bcš?ïØéf>+?vHÝ/&°?I)õëIõÆ?T¶HÛtÞ	?pf
r!
?sG·üÜa?ï{¼'Á€?vÏ´eÿ4'?cóhaM*á?\ šªê¾?Œ¶×ÒkF?t\SO?Ô?ïwS@™Î?eæmFzCÛ?mq¾5?N?ºÍ[?Šé/…³ñz?cL7'Á«?ʊ8?x}§v­+?h—[ö$?XW$…—˜[?†9k<FÕ?tjŒ¥"?n|y<?ˆŒ(9Q|Â?Y¹9\šn?e¥j
23?‰ƒ¨Ôe—?…½ÿ+Nc?îåQ°²÷?ˆúRD…?sµË-WR€?m«Æ'Ñ/?žnâý3ô"?…åž8¯o?€ÕÀ?¯¸äëV?'Sw¼4P?jB#RÀl?¡Aځo?~Ñ…õüAGN4FGL J0743.3-4912c¿°²F1|I´À(ÌxB0üøÀ:Lâ\
WÀ<	_¨Ý|@®Ê_	Oà@¸E܃#6?Ŗ^%Ð;?À}Ãû
?ùÃk$;?îDæҝ~?íÌ:5…óÊ¿å{¦3Ûϟ¿è!æڕl¿èe¼ÝÁf½¿ã¢©][û©¿Øˆ§ƒè‡AGNbcu1FGL J0742.1-4849cMRC 0741-4900?ïX êÀ?"Ôü¤´]s?d"®ˆ#?b÷C<n†ù?'|éc&~?"¾sGô?ê¿ß–ýÕ?¬ªØr?™,6èêþ?œÎ×DžBÓ?ÁО.ñ‹?Àõ;Q¸?íýº§–?šæó6}ï?…_Ã>?E¯v!â?ªÌ"?˜ßö³º©?æìš{×?ŸÜ·~ñr€?²þÃúG,°?dÇG*J§?ÊΟ›øTÌ?š"‹êli?î(2`qÒ"?£˜÷^°Œ?"äV-j'?ƒžD»$:"?© ãm€À?¡Ô²M=Í?ä4:ñ(ÝÖ?ÍÛ)«cà>?·<³úâ"?½koiõ?ÑÈ]ò'?ËH#|©@?ëŸæâoÝ?¦A^u$q?–ÖƟùµ?*?òóÎ?½KDY*?¤_¸*?ÙåšŦÏ?¦ŽÎW™øm?Ã!wf-?§™a-Ÿþì?܉ã+'†Ù?©ÌôužIMIXED4FGL J0743.6-3805?àÆzX"IVÀNÁ;ŸÀ:A¨@üI'À;Èu2²ô@Ó .^7@¥Q]À¥w?È-Ûõ‰¯?¸[&þWÅu?ñۑ¦†'@__ô²D
¿Ø"€}¾Ç¦¿åOì!%êu¿åUŸ~àÛ¢¿å›û©Y*>¿égõèO	S¿ïü<@øî"AGNbcu3FGL J0744.1-3804PMN J0743-3804?ïƒVÅà?"Xu͍˜)?Foþd¯è?5Ë]>,éÓ?Ã\¨ÐØÆ?"('4?í X‹ÁP?±WcR?Lw½Â¥‰}?YZo;øŒ?²ÄPW|?±0"¸ØOí?îEæ±ã®?–¸.2­?v…˜(ªìò?m3°•ŒT?¨ÐáìZ?•ÖdÃQŽ?ïeüºù7?lV‹ ZD™?P÷6_5Q?1˜Ñ7UÒ÷?'0õdrO¼?kox¤ÿ˜Å?îÓ«qÄy¨?™$º°¦· ?T'
ì.:?Fg51"×W?¢ ¸‰Ù9?˜üJM\þS?éRi—.–?Âʨk¼?^Ê̸¦?sŠÖ[˜?ÊzÂÅH/U?ÁðJ¢²êE?ì/¸™±cÝ?¥\ly'@¤?…Np:—'?{ö¢[Ú?»Øm)y '?¤PîõŠ"ê?îY&Žxíì?ˆÛt_—M?eVËJäþ8?O¤>Võ¦?©*g^hS?ˆ ýüo§®AGN4FGL J0744.1+7434¿Ûç˜RFÊ@='MÓØÀ:¾ù¥À<zŒþ€£ÿ@ –€
§Mâ?ÿ ¥&••ÿ?°¾ØmiåÍ¿ ‡ìa×OL?ðÂ0â (@7ÛÜ_;û?ç"5vÚQñ?d*®Ì©î¿åRÀâ]Ø£¿ÝB€Æ¿×1šânõ¿Í]v¾"eAGNbll3FGL J0744.3+7434MS 0737.9+7441?ï»ÀÊNÜ÷?mí±0}Ž?Uº–o:Æá?IJ	¤ìÇ?|°õ/c?jCòÖ·]?ï¾~÷	"Ý?xiÜ·®\?Só¡çâ£?XÊx?{ܼHÏ?t¨£ïQ:¿?ïg¹S·üË?ƒz…ª?aËBKŠo?_Ïɶª¼ü?Ïm>†sX?'¦èUú‡?ï ŠNŠã?vÏú®ÑG?€.£.S\—?^‰Ìõ'º?"×d¢¹J[?uád½N"Š?ïpïdãj¯?k»‡Â?f"·R¬;-?['t8my?Žøìúåp?~ß&٘0?ïXÿ˜|
B?á˜w4Þ½?gرZt ~?qÃE¦Þ"¶?'äöɧQ´?‹ÓªXûç?îÜg7ØŐ?¨
)þ
?oÈ^Ý?pÀ•Qº†? @¯ýÇ2?‹õÛz>Ô_?í\Ò´t;?'åZâo?˜´ýx;P?y¾ÁŸÅ?®&ú>Ь?'Í¢c+nOAGN4FGL J0744.2-6918?Åø[NŽÀ4ÇR"ÃÀ:'"Nü½À<E[sÄû@סçñÁ@œv"œ;?Ɨ–I­óï?°1,a¡Ÿf?æéHcF v@GÂWþÅ?ïû¬´('¿ÚZ[@B¿äü‹Rûпæå§#Å×æ¿éù>Dß-"¿ïóˆù8e¢AGNbcuPKS 0744-691?ïin|›˜3?´ŽÙQ^z0?a­gcßËõ?w-2í'ïÈ?œƒ~±(/?³—¯>ŒK?ï£ôœ¨w?} §-–'.?`Àùëúö'?bùº¼`
Z?'Òškw"ˆ?xB¥¤dWÔ?ï-ó³ÿ?ƒRy'"׶?s>=s/ï?pÝX%Ôý}?•qúCR?€#5
º?îù"/|?qš|ZÿO?|Z†Ñn\?XÙ¬kǼ?™Úå"cô?nöíۃÕ}?# ï?³–mÍà^?vÛ'b(kê?mèõÞz/'?¢ûúáØٓ?³?ÔVY?ïO0Ðéx?—èïŠjfK?q 픥4t?z¾ãƒ/8j?›MÞzâ-ä?•5Õ⻚¢?î5ß·yî?"ýÑdÄÍ?…ßØFhõ?(ç^Ú:#?§*?Õ¿÷?8ª@…×?í6z˜á'?ŒšsÌ:?'ƒŠjzèÂ?tp©YÛË?±ëLnânœ?Š
š\ôAGN4FGL J0745.4-2447¿âá¡°"\ï¿Ã<
ÍHÏÀ9¼1ˆ8HFÀ;]H2ž¹@¡Ž_S͈@ä4 ½?Ê>{eÒ?֋I?2É@¿)Æ¢ç @û
3\ó¿Ý9ÐÜ&$¿Ù†ðI©—>¿ìè®?Cî¿ê³¸þ¿ð?ï÷$ß³Y^AGNbcuPMN J0745-2451?ì'6èŽ?»ÿíƒâ´?—9>6²Éµ?¤ºN7I!?ºëݚ`¥?¹2ô}x£@?é%°§ï²?ÉàJ§‡Ýž?Ô~)ä?"a SÔÓ?ɗ`!†k?Ⱦ™\¡°X?æã9K?±AéÿEm?­nSÈä?›î¡òi?͘¾äh?¯*¯~®¡?ìç3#ÃÕ?4¸Tv£?‹Ká?qoæ™.ì#?µ^
Eíä¹?›F~â6«?çÝÐÌD?Ä'¼&âAÿ?²»èIN)c?²‡h¯¢âœ?Ç-ð—ñè?Âj©Ù¥Í?ßx.bÇ~?Ò*\Ós?¥g‡YÃCK?´ª
tàî?ÝÚà²n
?ђ,ÌÖv³?à!æyò	r?µô÷?:s?º3¾b?©þ?£±faUQã?Ù/CsŒœ?´UT¶FÀ²?æžy^?´ê&aÚÌ?¦É£7fÔ?'â–ƒQ¾?ÏÕYT@ZI?´iæ~Á|AGN4FGL J0746.0-0039?ïð7jFè@'©Çy¦µÀ:¾?A^o!À<4Ÿá²7@4,}·eÝ@ûÙ_'F—?ʵ'ž}¯?‰Ú5b"ÑÙ?»æ'ølŽ?û÷-Uù†¿?ïÎúnƇ8¿ì	XÙµé[¿ì½ªðÙòO¿Í~(¤äÑP¿ïÊÿ'¬˜$¿ïÿ9+
ËAGNfsrqPKS 0743-006?ïk(K3ì'?''±Â)£?‡»P5?'Ò_d½º?zõ:^ˆ'?zV­–½¥t?î"Ãtg?³ÝðM¿ØF?€Ï…äXù!?''v¡ÎŖ?ªbâL‹ªá?²6KoÙÆt?íXᢿ)˜?ŸqËwÌ»?–[ÁeÉ/?'Eh%>?¯f7ïêåæ?™£ò]áúµ?ïKïämÂ?xvOÓ(Ý?~sÛ9Zí?j ^)??Ê€lL?rèÌèêz^?în3ê"1K?«±?8á.??¢Ë«s7v?©Y½)¤e¼?‰DW‡v7‡?M¾À=Éï?ë@ì¶Äo(?×m\V??˜Ó4ǒ8B?¬'Í€"?¿ÃÍ@*µ?ÁO!Ñ¿ƒ?ëLNåÁ:r?¦"Æ´ôƒ?¢øÞhNË?˜ò©/'²I?¼!9áx*‰?£ñïF_»?ííÈd!+Ž?—Yÿ	fÚJ?™vÈï•û?s‹-"9"?¤h_…%?'«2 Î& AGN4FGL J0746.3-0225?KCùÝOìÀ@&a·À9þoï|$>À<-Ý­sk@ fJ%3?ü<`Ÿ±?¼àC÷ü{f?³Á# k…_?ù×ÜEԉ@	VcȧN8¿ï‰\:­Ñ?ïÿñBÍÛ¿ä!¥Õèտϗ¯I.G;¿Õw•ì¼¿ä¾pžM³gAGNbll3FGL J0746.4-02252MASS J07462703-0225492?ïä…¯=+?b§%¹Ç
P?5¨X€ð,¨?+uà" 
å?i6om–~?ao:¬S˜?ïËkrX¦Ï?€]öÏÌ?F
{5âŒ?RÆ5²SÂ?wˆ÷X¼,µ?~b#0:Á+?ïm4'h¾t?ƒHQ!¤ñ?Y#n9³ô?Jÿb"?ÇIýi8?ƒÎuˆ^?ï•õ-Þq?axÕÃ?YÕìd!|¤?<¢ñ"™#?‡H^eLF?`/¯x± ?ïÊìtªCW?s,Š¤Å?KÙB·³?F1nã9­?w_xg?qÉd­¿™p?Œ2¨Ê?"aø,Fæá?TLt~SVb?eÊd"èFK?Ža#¨É?"|ÜüC'µ?îå@i&µ!?'A"‰v?dºiF5['?a÷óh0ä? `RÛW»?ðiH¾Á¹?ï
½–µì?|Ïî?»8D?lxx¦À?W°´§2Қ?šÄ~".xð?{45\/AGN4FGL J0746.4+2546?ï¤ïjrP@6ފar
À9ºøW•KÀ<Ëùh6J@ó¿qÅj-@ýJ¡!?À2?WÙ°¶?П%ʔä(@	ÌDÑ	@ã$—9#¿ÖSb}£š¿åX&grÕà¿ìÅî Úk¿ìziR©ñ¿íeŠžT~¿ïý@'cAGNfsrq3FGL J0746.4+2540B2 0743+25?ïڄ«ÿUi?lÛ½Pd?bY"|$?_Y_3kŽ+?c!Á gBË?a"š6š?ïÒ¾Ä €Ô?vr¬üÀ?QÙT‰µñø?`å8cQ¾¤?r*HêÞ½\?pZ6Do!Ÿ?în" Ó—?ºÄ#ÀU?–1öˍ'k?'EW?êÐ?›û•·iÚ?"3˕‡i«?ïÛ;£LÔM?PáÓҊ²?Y^z¦«:??†ðE¾Ö?ht ?Hú˜j'ïn?ï¾ø•8È?{"K{Cb>?r¸´u=?oLÄ)<EË?là–&t=R?rˆÚ÷ïS?ïpYaù¢Ì?"\–ŠÄµ>?m^ þB‡¯?~yØ uïÜ?Œ'B^ ÿ?Œõ!(¥?í~g 3wã?¡‡AZ_?¢"ÆCˆÐ?™çb
N?¥‰4Í+?–Ó.0'
h?ï™ÐÚD§?q"ah© p?r°ìÑ·Þ¢?b	‡¼ÅE?€3S{àú?gî
Ö4AGN4FGL J0746.5+2730¿Ögníz@7|.º'®›À:f…8¹"ñÀ<ZÛýÂ8@Wxð+̍@2³Ïà?È*2	h?Ï/՛'Ž9?øœ"ê-/ä@
»
±‰ÐN¿ä¿ôa¼2¡¿ÚPfíÖÞ¿ê
d1Xh¿ænd!¿ï­ÞA¿=¿ïã~õ©déAGNfsrqOI 272?ïÁ˜<eâ?rþe'SC½?[v)[ÿ¿B?Q:ö­e8G?xVuŽì§<?q[À}©d?ïÒh2¡ñ`?vû*©Yÿ?QcÞµ°T?\× ùÔԘ?rrï;W´
?q:¤[1†?ïXÐeª÷?‡}ùzáºÉ?v9+;‹P?v‡§\Xy?Ž¯Pÿ»¦N?">MN;?ï½—¶·Ú?Y?˜«	éñ?bÁYÖ"õm?C@i*?x"å,r?TPÑÛ(U?ï|Öm"	?†&Öy6S?i1u~ié?cé'x»š?Š~HÇåŸ?ƒ×pËRn?ïu¸¸æ~?ŒhÄ«c?c¸Ã ¿*à?p;p ¢0?£ ç=QÊ?‡Ù§Å?îZ!šÀœ?•ª×‰³*a?ˆI §··?"òd? ž*M?'ìþf:?ïIž`¹å?x"˜GEý?xÂù5GÌÔ?b\OË%u?®ïÛ?sÏVåI^AGN4FGL J0746.5-0710?ì¤ÍÿŸ)s@! c¾ì9zÀ9ùÓ'é|À;úPA`ó`@µ¤ÝD"/@»;ªÐú?½_ÎÇ£Ã?ÊÛ¨‡É¤@V4êK@ÑâgÞª?¬MI£¦Ò¿â#BzMú¿Üt»(_šš¿àó 
Ì✿éÕùœ8°K¿ïÿÊ ¢¢WAGNbcu3FGL J0746.6-0706PMN J0746-0709?ëwÉ¿jþ??²³ýö'?³1lK½?¨Fwsb?°´€™87ä?¥*•%§ÀŠ?ë9Hä
#?¾ö÷ fŸ?™ç~F/y?"4'jvB?Á¢½?¼>?ì)3€?í¥ <dÎû?‹ž¼ë™œ?œ;‹ì$7?'Û#*;7Æ?§ˆ6«å-?"CÊU[ˆ?ìèË	lÿ÷?‡7Ì¿`Ó?—Ÿc ûg?r|i\ð7?²ô݇i?'Î/0'?ãÝ3'²'c?Ânµ_ÊV?̼ìßé×?ºïfÀ(yœ?ÃÎnWxž?³Í­Óèhí?ærÍ8Ç5£?ÈháQ$q
?£OVM–@1?¨,â)]úæ?аzÄõÆt?Æt2"&È?êÔ^$w?«»cÕÓ¶À?±1{WåJ?¢k½‡BPž?¸+"0㝀?¢&š-<?è@5¾í€?ž(ÿ^·žÒ?«
# áw?Šöþ«jr'?Ç7¶`àÑ£?™ŽvÁK'AGN4FGL J0746.6-4754¿ê€ù`dÕÔÀ&œYyÀ9¾Ó-À;줾Éç@i*»ëS?ÿØIё?«Ý`\¥â?°ºž¡ì#@"8T~Ý@Ö2ÊÁ?íÐH¢†'L¿à‡·ïÅö¿àÂ_
§y¿Ýe¯¼ñv¿àUó‡K¹<¿ä®mє²ªAGNbll3FGL J0746.6-4756PMN J0746-4755?ï âÀ¡g¼?—ØX"ži?@:îtrø?BŽÌùý¹R?†Ã¡ƒ7ä?—¡F;l d?ïÜHÿd?{'J80»?8¬iÃS¡?F‹1 Ç?pPº,n?zdo€•`€?qKÝ?ƒAz—"õ?\àiaksw?VÛ¡g ?‹u֊ª'9?'ã3Åyy?ï'Ô—W±(?f,œ?\X¯'­Y?=®}¾eî\?‡¿ÙýÀhC?d}ГÀa'?ï~m°K{˜?ŒNjºº?N.µðŸ)?J½Þˆ2ª?Ž³µ(à,?‹*ûÃ7?ï"ýÆö?'úqgú¤Ç?O9¤*ù`•?`db/;?ˆÌô;°î?')ﱋû7?ïBC=[D
?‰ÎRc5þ?fb¬
Š».?gÖgW^€?"ëBÊ#%ÿ?ˆCt"´?îâÇè?'èÖ›°?r®y)Öv?X×q–Na?Ÿ:ÑؽUg?–Ní5\AGN4FGL J0747.2+4529¿æRr0>À@<hpdìé£À;8F:vôSÀ<½Hɝm@–•-NB?ü±'<ÓÅå?ÖÅi–œ?ÒAIvk—(?ýËûf=K»@O_™m¤É?îi* :8?ïÑÞïäÿÉ¿é¬ðžŽ ¿Ã`–‡f¿æ»E»Ëó‰¿ïù!bü$AGNbcuNVSS J074654+453231?ï¶H¬A<
?sƒá5ŒlF?Zõš¢¶Tb?QŸõ—³ô?~CW°¥?q¢XHÛ)÷?ïªn·~î?yIzÄؒ?a‰!Îì–?h
‹†–ë?cp?zwÊ)û?ï[¤f¯¿ÿ?'ªO/LM¨?j3'&ÿ5d?cjO= »?'Eæk?dÇZ$?îÁª»'!a?€ù£•Qþ~?‰Øó}Žì¯?rÅ꣫úó?šÞ.Ï]'?zEjN?ïŽ#X8•?|½ß÷t´?j~‡Þï!?bgRë!†?…ׇòÅ]V?y krÑA?ï¥kù'?›ÙÕà!n?v•Ê:ùá?…²lمŠ?–öøÌ-`N?")´}8?îÖ¶©†ü?Žá¾ò$½R?w­Rœü˜Ì?u
ddØ?Ÿ=Ö&1U?‹2wð~7%?í.Õ¼H
?™úå¦+†?•ð¥Bdìx?ŠÓvÙ?±
(͊ª?–+'ÕºKAGN4FGL J0747.3-3310¿ïüóIýêÀôÎf*…À8–·$¦À;J®ö"0¬@¦iÿÎÿ@"œî¸°?©cðüh,?zFäÚ¤j?ч-@´8"«ËË¿»ëXÔŸg¿Þ¡MÃqð¿æ¡wI¹L¿áÆy³JE¿åsUb2$?¿ç2¡<ü
AGNbll3FGL J0747.2-3311PKS 0745-330?ï«p
õ¯?wß}†ß?9[þ1<K‡?+¸è@?"Y€«û^?wt'(Z1è?î¤D¹ %?ªífΪÃD?:L;Nw4ø?P4î§ûRj?¥Š#<"j?ª¿Hœ$Y?ît•t'1?™¢‹Z¼?pk¹m9¶O?xXÁðu?¦©1Šc1-?™Ôºw¢³?ï¥Ù2á©©?hܘ;‡æ?DIL¢·z?("R
?…@Þ¨¨'j?hãH?ï)SGÈ
?IA!ïô?HDÁí»?;€¦%Dm*?šf7¥/e?
îÐ䦷?ë×râÂú³?Àt'š"Öo?L¥ÎcWŽ?hf^@Ͷ?À…mé	?ÀeYØÛÆ1?í{gs›?¡ Ók ?}~Š°¯?€ÍÊÙA¢$?²SîâZÚ? sLDO…ç?ïçKÕõ?…t†ÁxüX?_Lcp5õ?M?Fv«?š®]*%?"Sd½'®AGN4FGL J0747.5+0905¿ë&$	–ú@0zÝð,À:|]Îè0À<€ß©HcF@§e3‹rº@
Òä>š?½ëû€]—?¡ôsb€Ü<?æÃx?ô‡—5秿ï±×~¶ß?ïÿ´‰	)¿ân—²8Í¿âL^G³ó¸¿Üü³Ú¸rοÞüR@¿ÊAGNbll3FGL J0747.4+0904RX J0747.3+0905?ïmúéâÿŒ?'ÿqñ§%2?\z¿{jÙ?S_ºï5r ?y5Ďä?'¨Pµ‡ÞG?ï"[þrP?šÍöIb?yær_uàÈ?}c'Š*‹?•E—並Ð?–'=D¹U?ï‡ü
W,?Œ)¿yϐ&?t(j*^Ùð?u>uûr8?—äåø`Ý?ˆôS; ÆÞ?íØrã!wõ?†÷©hpa$?•÷â¹Ãç"?x¥!'çõÐ?§|ànr×ì?' qÃõ_S?ïÉbpHÏ? ~œ
g?p…P5`Ó?m|8²¢?˜©€ó? I‰ß,ïÏ?íƒGí`Ž?±ÚÊÖf?"ZtÂq@?¡ ·»°ª3?­ž@tô¥'?¨—¹ay8?îMŽ\_ã|?–ÔÍG'#3?'Õ®Û8¸?é;»—p?¦q®ÓÂD?"ü‹4Æ<?êð¥4L?ŸjÕéN?¨(
ʟÊ+?'eã†8?¼fÏyǹŠ?›Á;Û3©AGN4FGL J0747.5-4927?ݵ¡`ý	ÅÀ'ÑÀ¨ÒÁÀ:®rn²À< Ô¿ª¥@`Í p@ÍüŸù/+?ºšÒSÊW}?¦è©C¨Ù?ï˜ûC؜å@0Ûê÷Û¿àæäÀßXÁ¿ãQL=Æ4,¿æՒn,-…¿Þ¥€B/¥_¿ãì ¾üÕ¿éÙRKý."AGNbll3FGL J0747.5-49272MASS J07472476-4926332?ïz«âòS?"ÚnÏU8"?[pEA»|¼?Q*…0Ì;°?æþ¨ò:
?ƒ^Cæâ]:?ï Çö¤6¬?‰å²bï±?D"+ì­S?NlÀóÕ³?†"Ï¡ØN?ˆùéâó"æ?ï?N&å®?Ð¼ö1÷Q?i^gðÑM3?\›ÔÇ'?"ñ©B\…?½S_ñˆ?ï4UךRž?nÝdóW¸?oÆFÁʁ?Jpjє|ÿ?•||:S²?mEzíãÇ?îº`nTÇX?›ë=
B+ö?pæû´°8?aøѸûÑ?¢X;hï?š¼SF½Ã^?î´i> ç?­ÒUÊMEÍ?WUWä°%È?a'Ð&Émr?¤n¯Îâ?­¢d®ÖAÁ?íä®ÁQ¢?š"õF¼È‹?ÖËPç™?s¯Šk,4™?­º:†¶(v?˜-"—?íÀïns?‹‹ñÕÊC?‡›·oÝ!s?nžØo°£Š?®
 ÎÙKÉ?‰©»,D	AGN4FGL J0748.0-1638¿Ã±zùg×Í@Ù½¥è\À9cÆOJÀ;´tÇR9‰@Ê·ÚwZU@LԁÌô:?¶iqž'óº?ÃnœÊPœ@xq¡šð@f'ÞdNß¿ÇûĜ|¢é¿å#—ŸC|¬¿é–ˆ¢ÑPÀ¿æŒ¹6£*¿îT6ž!¾—¿ïÚ¼i¨:AGNbcu3FGL J0748.0-1639TXS 0745-165?ï'ó¼Ë?D5¯Of'?m­á'bî?n'ˆ®'ó?"˜Á6$'?vº]HX?íöJÓš?®ýø`¾?w"í93:[?€èÊü®I?²þԊE?¬ïï¸Egy?ï=Àâcb?‡g'
øÊ?tL³|±?r;Xáb™õ?"FœÖ촔?ƒuÕSñê?îª~á²b?wÌjÄÊjâ?†§=jExm?bӋeëá?Ÿ\…Ù3~?sÈ/$¡ó?ï0ÍÆO8?‹Ú÷^¦'??ô	G?z÷¯ÛĜ0?'aס4?…o}ó='?ê\#>Éik?Á>r'KÆ?¬^ÖÃ2?ŸÌðN«5ƒ?Ĕ­û`?Àrf9oã=?îºÆDÈ[ú?"(øüée®?ƒÕÄ|Ÿ?€ÿÀdë"K?ž¼³Ó{?¯øìëo2?ìSfUU?•$Ú¦p?¡yüÌ=¦?"bƒe¢1ž?´§Ñ® ?ÄÄ*AGN4FGL J0748.3+8511¿êžGœ@<5‹¤
âÀ:´úȈšÀ<"çä€G¹@ ¶–*´Š?ø+®9cÎÜ?ÀOJ*›Š
?Ç
¸À¦@	ßøØK@ó÷ƒ¯¢p¿ïÿñ¢o+1?ïþ©ôZ°P?Î\u éY ¿ÐÐFŸ ¿à†é~3a¬¿×š¤ÆôE¸AGNbcu3FGL J0746.9+8511NVSS J074715+851208?ïÅ8ðÑ'¿?qY;-D0,?iÈl"bŠu?cnt±¡ ?pQn-—T?e/&,NÁ?ïÈú~ЄV?{•t ­¶d?UÒK^ô'?bH"…Ea¥?vÌ b÷ ?t%œÂØ?ïX‰rÊ?'F ˧ˆÆ?t¸
±1n?y¸ÌQ2?˜Qт3än?t¢ÜfÝU?î¨õö¢ðA?€{Ÿ@ÌÅ?y(6!XÏ?]H—Zb?¢Kž?^?~
WM+?OçÒj?~em"?wÔrjLU?oëÅêêù?zäå·Ig?sQôÄ)'|?ïY úO֜?"¤2ë2ë?jchÞzo?v±wNȒd?'ŠôK}6?Q:9Ÿ¤o?îQ¢ÎeÝ?œS-ýî?‹	YšûïO?‹UØß²½?¤#‡þî[^?–s‰IP3?íÿž)?–bCWr̉?…íõ*RÓ¦?u³®)«?´'9^2ŸÁ?•ö"Ží©AGN4FGL J0748.3+4928?ìóGT@=AÿÅGÀ:µbÙéëÂÀ<Žn‰J—@€§i»Ûc@ü&V«Þ?ɝµÝòå?ÀçàúVGà?ö懈õÝg@²ê%MA|?ën0Ê£&á¿åÑ£€ùÊ¿ä¨ßá¿à–Fދ¼¿ï¼F¢{Àk¿ïZü¥Øl=AGNbll3FGL J0748.8+4929NVSS J074837+493040?ï¿O´‹?y,T*§Y?\>ðпû?Wûi܃?yIˆ´òn?u,†2–û?ïÍu,žS?uª¬Ó¾q«?RQVÛÙ?\½ÿîøU?t±(½÷t?p+ŸÒ	Z?"‡È?zò¤0¤8?e§Â%MÈ?n5²tÑ?"Y±sRx?u|ýeË©?ï‹î{Wª?dç©xÞ?uQº6bÄ?U1ƒ^Üg?'["#Ph)?_wö<Ïí?ïU½|«Tá?‡ÚBäüÐ?t¹…øŒ]?qþ>;$pY?ï.:iÍ?'ÚXáK""?ïrtÇR9‰?Š´)…
E?diÿÙ¯«I?oØ3ÓÚ¾?ŽHNCì?…û¢Pã?ï:G|Éݸ?…ôĝ[z?o!;®"¼	?píüŠd#i?"ÒèõÁE'?'ü(Šßê?îÌ»ÙÏ-"?öÂyj¯¶?‰Û@ü÷_?r×íï¥Ä?™zäN}úG?z7É\¸7HAGN4FGL J0748.6+2400¿Ð'·Ôî@6»³"ý*cÀ9T²ü(À<+%üéË
@ñ~Ý֊@S·RDÌ?²J¬azŠ?¯JŠ¹'B?÷ëýáAÏ@³a+"?áÓ¦¥ñ–±¿ä& !]ž¿ãÏâÌ'ª¿ã©&4G/i¿å'«_ê¡I¿ïÿþR€ÖTAGNfsrq3FGL J0748.3+2401OI 275?ïõ­;ëq0?Bwi'D?,$(-?Å~8½_?Q"ÇôT‰ó?@@d)÷ç?ïçb\«?hËã²?;…E"³'`?IïߧÛk?esõ#7Ò|?d[DÄfµ?ïÀW0ñí÷?dê{²cÏ?Vþ²
0ý'?T'ÉõæLT?z»Ù?_×Uå/ß?ïïÞ{º¥G??^6ÛvV?8éBàÊ5?,ç ü–4?Z¸@¼ÉK?<³7˜ÿ0?ïïaŸ';Ú?O"Žäš?7<ä¾Àà	?''ÂXDî6?[mˆx
*?LÞ‡ÀNr?ï¶`a"š?òÖWØ2?NÑÜ ã™?_Žójöº?€zÉÜ?Îý?}øÃV§È?|¤Q•?x^ÙJš?eAè6ÆtÉ?gpøÙÏ£o?ˆæÐq+˜?sݱè˜ã?ïÔ"ÏìD•?_žá7ÙY?Qkª¿"?;S#h&SÆ?q"­£ê
ü?[ë0"g]AGN4FGL J0749.0-3904¿ç¨/¾«ï)À†?¼À:€ø¿™ÞcÀ;üFñ'@ 
=Šzò@+}\L1?È	<¿¤?²¯«~É^®?ícQÞïå?û½Ö½f}c¿ï`À¹n ?ïãÖ3}Ûοçxâ>ùæ¿ßøelkc%¿á}h@[9â¿ç
¢µ¢
ÜAGNbcuNVSS J074915-390336?êòûEí0?´0'²äQ?jÇ+r?Uõ¤
¼-O?Çø§úŽ?´ •¯Me?æVA6p&?½á¸_`r?xƒÎÿ®¬?z㊭Þ?$?ÒñqpÊ\I?½ŽY'¡
…?ìâJɎ?¢ˆ' :Å?ƒÔÀŸ·|Ä?u¢2~‡6l?¼¾U"ö¶o?¡õUk½v?ë»*½».a?'"»Ã¢ó?rÙ×ÆQ¾?q–ßL ªó?¾	óš}*‰?'c/)'=?äf¦¯¤
?À¹äƒ³å[?v<%ÿò?c¹àõmfË?ÖÙÀ-à–Œ?Àº}C;'Ò?Ú±Æ×â?Ãꉰ1Or?"¨ëë!ÖÒ?—½ËKD+f?âTœm.?ÃǪ%Á?åìéŒv?³ŠÕ˜ ¾T?"ùmŒò?€H?o½'?ÒæL–—»?³ðî{Yy?æ&.@7Ü?¥mÜS1é"?¡7¬°öÎ?‰þ<žkæ?ь­è±î?¤ÝBlµU¥MIXED4FGL J0749.0-2956?æݍ.ÁÿÀ[íœP-?À:…ôÍzÀ;ނ€x`d@!$ÎÏÜKÆ@ŒÝÉtS?ÌÚväãÅ¿v«ÛKÑËË?ªŽ' cµ?øǟñøUg?؝¯]¦#k?Åíxé˶!¿Ü¤·$D
¿æ
š"U•^¿À7œ¨M¿ê¾;Ú¡¡¦AGNbcuNVSS J074913-295658?ãa8ôµ–r?ÅÂÚ
Zº?p¥N¸-±?d¹ôä1- ?ØýwŽ,u?Ų,š_3º?à­ ×]l?Ê>Š›56T?~nÉÞ9c?ƒÂ|3þšZ?ßdê–Èj#?Éáu«ëè?éû¬x×Ë?¨)䔢`?Šp*†ý×?€"®ÜÆòÈ?ÆjKtíV?§ŠUj%ôÂ?ê˜éÉ4?œä	¸6Ê?~3,ƾ0?iô1`?ħò
Q›1?œÖ³©pÐ?Ù9¦!´¨?ÅK—`YS?xPlw(?m§ñ°û?ã2ÔÔK4?Å`Uú¢6æ?Ñæ@Á'/h?Ä3¯«÷k?xï'Ç}%?…-_rÒ?æÛœüš?Ä*9¼†¥î?ãˤRôÖ?´3öcGmÀ?•º®ûºþ?…¢ùáû)¤?×
'ØN$?³æ%HÅÞÊ?ãrÕÊnÅþ?°éKsÇ?‹°öaÙ\?«u£ê?Ø<Ì·Ü®J?°ÍážæÁˆMIXED4FGL J0749.2+2314¿ì‰Ùö´…a@6–Κ,fÀ;˜+ÛPÀ<ÖÖ@ ÚêYûsÿ?ÿJ¹t*t?Ä#ÛýA^Å¿"=Ý8ÞKƒ?ÑÚ@þ¢Ý»?úñ¡µòÀ§?í8"ñœî?ÕHÒ¡ø㬿æq®ÞÐ/ƒ¿Üå<hš¿àO×äXÍ¿Ðq‡+ØÌAGNbllRX J0749.2+2313?ï²ÝJڀ?q¼/]'8?NÙ-¥ä?<ª"ÃZÏ?õÝ—Ô?pÎÖ2ÃI?ï3˜ô;?–|b?ÿä?sV"a£jr?tlØ€e?"·Yðw¦õ?"šs–øÿ?ïsØ«ìò ?x[2«ûÓ??d8€h/ë?^lESÁP?Ž†ç&?vBò5r?íþ-äY~?ŠH%VÓU»?‡X:ÿ…[Ê?há}=­\‡?ªG"lÆ.?‰ît:°D?ïWÜ3áÈ¡?‡©²©P"ð?]Ž±–3X?MRAË«?"+Žgüˆ?†¼ÃjM{´?î&]`>•M?¥ðë¾i, ?DÆmŠ	•?…w³Ç–w¾?©HøcËÎÂ?¤$$û̏q?îëd"¥ƒ?ˆëȋU¦S?o™šD¶$¬?f
n½u?ž«@,I!?‡5ŽÄ%?êlԂÏ?¢i~ã¾^?žm)B&g´?‡÷'W·Ë)?üª{û4O?¢vž¿^ªNAGN4FGL J0749.3+4453¿Œ>åï!O@<¨1zÌNùÀ9ݍƒá¡pÀ<sn]«¬Â@"'Êö@o¡—Zû?µºµ|Ô?À0µS^w@c<æ:\@
щ5ô-º?ïèB©È»Æ¿Ý꣢\
î¿ãÔÖáΑž¿ä†J!aN¤¿è ÈÝ~ö«¿ï÷½ ‡_AGNbcu3FGL J0749.0+4459SDSS J074916.88+445232.1?ïåj,]p?^`5ÓT.?Gàe§ïÞ£?A²[އû?e|7|L»?Xž¹W麳?ïĪt:î?zOH›Üá3?Z¬74d?dørÑ®?wIË?r©ŠO6ô?ï¸Ô1gx'?m
Óýõb
?[;×ä…?Sn¨zk)¼?|Çœz
?ia^Ð'Å?ïšzb?`<'nÝõ?w¢ÝŽÄ÷?SÔÒ-Hˆf?{ Gl	Å?Vƒ¥†Í½?ïÀ°Z»/?rJfoέ?c߇?Ó¦?b^ŽĊS?u¸<bþ?hý¼9ôÆÑ?ïnwœ;+ò?4~"­3?h.îo| ?sñCÕ¼èX?ŽV]YÍPÖ?ŠÇH÷?ïv‰ž¾ã?"‡‡ÿÙa?pÑC‰?pkY/ë+è?ŠS¯ê
ÜT?{›m[YŒH?îì&?~E¤‰§D?|¤a
ìI?pæÿÆ#,?'¼Ïú_ÊC?u¿Ký%ýbAGN4FGL J0749.4+1058¿á%¶¥ew @1Î=ÁçÀ:*GÒ&©À<J.oL@Xž¸ge@ø¨ê'?¸?W?JÂ?wâ?Âç?ÃÓ8KËÛ@¤©Ü‡ÕÍ¿Ñt
~^)׿ç¼Ä¬lÚõ¿çi'"š\¿Û/[ßyοæÀÒ@Ìú¿åâ,EhAGNbcu3FGL J0749.4+1059TXS 0746+110?ï²F¥< S?s6à×Á(?Uc!QM>f?@÷Æà
£?€Áò‡Ö%w?rŒÏ'æ9?ïÐâiD?u®ß7CÊ@?N'aîÙNR?WÞ0ˆWÙ?t 'Bþ>?qKЋ¿ø?ïeÕ{ê?|
Ä`?i/Û¡:Ý?e4µÊíƍ?7¡³Â°V?xGuþ"}#?ïžUyã?a—cL>;·?f\B‰¦?EŒo‡Á?'ӝºÓ2'?^íß tZ?ï%"etgË?Ž*ç!qE¼?i‹`[ãh3?W
¶È"º?˜*GEF­¥?
«H:?ïv'unþ!?ŒùfþÿÎ?^HyÉǖ?j«Ò†'ù?Ž'Ÿ þÎ?‰°/£\	?î"ꄇ}|?''YÉ¢?|†xÖÞ¥?t^…Ãå!Ì?£ ˆ´5›?È(¨^¼ ?îèTá{½?'BМ©†.?…sáàf?gº+m•§k?š2ªLDQ>?~‡ø¥ú@EAGN4FGL J0749.6+1324?ïŽkbF«@2ÝËݹ"À:űg¸ÏÀ<uTZË'±@·‹òçê?ÿb¡e?õ¹?Ð@gä•ÁH?àsNÁ¯r@v&}BJþ@Sò•í=¿â·îÿQ¯J¿Ý§!ïi¿Òo,Åǿ敏~¤™¿ïûæàõ"׿ãJ½É#ÊàAGNbcu3FGL J0749.5+1320SDSS J074935.95+132156.0?êݏìWè°?³âàÀú¥†?´9-´X?¬ó9·Ëw§?´ÚeoN%?¥ú'MÞÁR?ëd"J8D?¼++tDm?·œVD¿©w?µwp/˜?¯a3"öÕ?¥¶Ç|ž?æ>×M¦ž\?±?‹?Àˆ'?Æ`:?¬/,?ÀÿB`ty?¤¸þ÷‡Ú?ì{ž=ð?"KޗþÎw?©&MÆÔ³?†²Ã¤>•?³AgË¥?‰éÑóàß?åì?wuhž?¾wû'J{,?ÁŠ©¢âSÙ?³œUäø|?ÆÄXH	¯?¶ÔĨf*?åV~0 s?É26B $Ò?ÊÛð^ÕÖê?Ɲ¼\äá?¿"-Ŝ=?±ÁƒàGD?߀´#Y?·Ÿ€Óü?Òþ÷ýR%½?·'Ë­¿ §?Ëߝ"Õ?±
AO},+?ç‰/8I??§DŽ"¥‡2?µ­ÈTr³?z‡ŠÂI
?Ç_Â×?¡×ó%õˆAGN4FGL J0749.7+7450¿¹öΗÁìä@=éSXl¨ À:ð‹+AÍÀ<³ çTº@ )'_
ž@N~:˜'B?½ÿ ‡	7¿®"ä¼é¼?ïñà'Œ7@ël‡è—.¿á!‡Ջ¿ì·¬ª–¿Íõ:ꌦA¿ä¬©áæ9…¿ÐîqãD"¿ê݃¬8XAGNbllRX J0749.4+7451?ïˆo§IÓ?™Z†`=?Yœ>:©nV?h"<Ãe?Š°"C)±?–â!‰Þw?ïÆӊ<j¦?tÎî«:÷
?J¶¥ÂÌF?PñÌçžè?y?fÊ°,?rWN
o¹?ïDBÛOz?""=çG?`/h®VHn?]9÷ÏB?•q·‰`ê»?ƒ4ºÓ³?郎KM=?g^<`Um¬?RŠ[Åm?<srp0?"'ÉmQ$%?g>'c·VŽ?îÔ*œƒ?~˜QêJ?js{Þ)äÓ?_é!!þÏt?¡'ø+p?œéç
5Š¶?ïh/R9D?»eÿ඿?[l—©§Ñ?g'4I£*?'CL6㌚?Šk	æ?îFeêbs?–þ¸Ô³¦)?j@cT†'?júPxj€?©õ›'W?©?–©ÊÓÉ!d?î¬Å¾Ä)?Šÿ\SI?m¹Ðª8?aÙÂÚª¸Õ?£X)â?‹:ëëg6AGN4FGL J0749.9+1823?ѝÌæV@4ëßÁœ"À:eËΠ¤À<ÑEØQe@w–÷Cï@ÀXeã‹?ÂáðöLÍä?¯5z`Cb?êæEy†Ô›@	7>$þ½
?ïýU–4ŠK¿èž¿=˜¿ß×µž‡êð¿ì0¯?ž%š¿Î?|í'hs¿ïÿÞ˜–dAGNfsrqTXS 0747+185?ïÈTqz?s:üó^›'?KVù¬¨?D½sH÷¥+?x™4‰ƒå?qòï	YcR?ïÉbëÃÄ!?'y®>¯¤±?Qçøw¢…?dƒaM¿§Ó?w
P@LZÓ?|ïãbÈo™?ïGHoõ@?ˆŽcfžóà?oQîëZº?vxwö/Á?",´Déߚ?…úºæ ?ï¾C,%?^Ò%Ÿ÷T©?B±<Í
?.^ÿäÑ1?~±ê6'Îã?]}²ÜÎ?ïn©ì֋?è\qÜ@|?aÂáË9_?`bŸ¡ŒR?
J	M+Ž?ÑŽº©?ï|[Ó»S?
L›JYý?_Ä4ø°*?n,¨œEÊ?x·?ˆ1tML?ÃÞð?"bиGbH?|Ï:ñ.µ,?€ãF›ûµ¢?¢ºŒaÛcÕ?'ÉIc
S?ï=Ê*Ûö¶?~›ðŽVp(?Y7Ï3¶9-?M"§±:eq?–³=²ý" ?}bÒÉk7iAGN4FGL J0750.8+1229?åŽÀžQuz@2¼… ¾Q	À9g¥‡À<E8ï4×@à–ºìûk@äǕU?°Â5o"¢—?³K—ƒñ$@"ºkáÐ@.Ó8¡²?î¡À_@˜¿âDÞ¥gX¿èŸJrÉK¿ãÂð	è·¿ëÌùÆ·à¿Ü¨ÿéåAGNfsrq3FGL J0750.6+1232OI 280?ïð–"L'?L%
¸EÈ^?@*}MK?,°Dðúá?V½¸ÊÆ¿?HmvG$lÊ?ïâþÿò5‰?oáÅ#Øn¹?Cuøÿ—&?QH[8Šàï?h#˜Ï,î?i€HÑ]ë?ï©á`æ?wx{Ér?a{v(ˆWÐ?byÜS{*?(Þs¥Ø"?uKyÛûM?ïíÐb%•?BDÐñ00?GÝFÏ,õ?0NuÊâb¥?Xp˜3µ˜?<-+æ]éð?ïè	͚cT?[(÷µÎ—t?KÝóȾÖ??ò22œ©?`þ뮓i'?VôI¾e
?煮â½$
?…˜"djE–?V'±´íæ?fÌ2åÜÆq?'Ë'*¸ó?ƒ,€µFÇ-?ïV±åd?‡2PÇ^…?r1‹ÌPò?tg åñ"ƒ?lÇZpZ?"Bk}o?ïÇZß
…é?cȟ\gY?d":K3¼¼?Q¾€	và€?rsRó@ú?]·xs&AGN4FGL J0751.0+7908¿ïÜÅW¯á§@=gT~–À:ŽàùÀ<ƒØž'&ß@n"ˆ7Ç?ÿŽÑõ*¹è?¹.fDØw%?ÊOʘ•Â@ m֝0'@t—>u†•?ÈA•Ì…0¿Ê³!€nÅ¿á	}±Ç¿âÌËN¿ëB‰Œ¿çŽd²1@AGNbcu3FGL J0748.5+7910JVAS J0750+7909?S0‡:?º&,fœ¶?"_äËà€?}¹ê=F?qô®ˆ× ?cDÑo¹–M?ïÛ¸ó|?qŸ¦ºó",?I3ÄÅÄ?WqÑ<"Ï?mú˜'æ?k|¥&D7?íóø³Ž
? œ$àËa‡?¥Ä¥ÉÔ?›^4{Q?•÷ŸNÞa)?<ƒØ«ìò?ïܬôó»?L2±
npH?RžJí‡×ù?5uhãrnp?jåÖºÚ?G%­––Ú?ï7ÄÁ ØN?Œê8pvN?'¦§˜6¢f?†ìt5p ?}ƒ%f»O?råKÐ̧?ï'ý'+?‡Á:Ï2"?\½4Å)Î?gëbe® ?‡ýgËöv?ƒò5Ñ@úo?ëú÷!ßù¥?«†)$f'¯?·f¥;ߺ?§«B¯:?¡ƒBÇÔ)2?"™‹Po?ï¡&V€ë?kÕrý¿Y*?fQsúJ?Q"ø'™w
?'bLò•?g9&k¿`¼AGN4FGL J0751.0-5131?ßå,·e~×À(Ç\¢˜FÀ9‹B¾ÁqÀ;µgôÛߏ@ÅûI{@mÆâ¨e?®Ðó"!?ÄrlN'@Dä]ã
&@ØP¹€ë¿Ò7¡¢&°ï¿ÝÌÔ#Ù#¿æ§¾ aŸ¿å`Âl »¿é™QÀg
Ö¿ðAGNbcuPMN J0751-5134?ïÁ"/Wº?rŒ%8Xìí?p«4ðüC?e`E	Qfë?nNzIbÛ?e³OËà'?ïêÏ<qS?mNükŽ¬ö?1ü"ü€è?C.RÙ¿R?bñ?YÇp'?jýQ­"^¹?ï}í©Þƒ?†5èý×r?vխ͏?~79û?…O.:¼?}­¹'Wà?ïðô¾û A?A¨·_9Ô*?'Ïk¤RÅ?å)ÿ?["×Ü)?@jVKɱ?ïrÉö{i?ƒ2Ñn‰(ë?€Íÿûfú?wº²`=l?''ÑßæÅ?wXøÈàÐV?ïÊiðÜ)?"=<Æ4Ð?Q™™7¾?t
Æk8¥?vˆQ;g¥M?€š¤ýl?ï*kºtkÉ?'\€v—gä?Û"Ršd?ƒm8m|Ö¥?'Ä¿´xÏ?‰·bYáH?ïÖØ+/Ù?aB=ÇË®?AKK´¡Å?4G[c``x?rj€Ú4"6?`TÐÇCWAGN4FGL J0751.4-0421¿æáÛ4Í×@&¨?NÊhÀ:v6¾/À<k;÷'@k•\É¿?ü5g‹)"N?ÐKÚ®?ÑjÇôö·'@£øôõ
?ôr!èÝúr¿ã™µž2µ¿á1†:A¿Ôy_ã•f¿Ùýh
«T­¿ãí˜>¥­#¿ïÿêњ'çAGNbcuPMN J0751-0421?îöÒö˜´S?"¶Ï=~?hRƒ'"•??d¬±…eÞk?žP¾^u?'î­(^ò=?ꪺ3 žú?¿ãucb?ž½êÍ7©?šî1¯?Á}YÙ ~a?½6×霢t?íÖsñƒ)Z?›ÿÅöÙ`?Óâ™&|ø?Šªý"º?ª.Ϟ©Çç?–ï\Š=²È?éî&˜}:?—)'>2k?¢{ÄnõÐ(?€ÏŽçšžž?èv;©Ï?"rÙƒœÂ?í^&&w?¬®‡Âu"§?Á¿O!*'?{ÆqC…*?µàòە— ?«j'¼â'ê?䖔‰ïû?Ë,1_&3Ï?²ž-qxg?²ˆØÖ+?Ò+KÕ®P?ÉÁ`_2·Û?ëÇYÖ`y?¦tøúxÉ?›×H˜ùuG?'î¯Þ~?ºÏ_#Qí?¢àOnNÓ}?äÇçÆß^?ª'÷(¶š–?ª°)
2`?'ý,0͌Â?Ԋk
•ù?§°ƒÓÐaAGN4FGL J0751.4+2655?ã\TD®c^@8Tòù‡@À;fØ9¦ëÀ<ÍcЉð¯@; Ákš®?þ'¨¸]ª?ÔÙÄ❙ƒ?ہ¬]@¢Ý@Õ™Qu>@¾ù:!E¿ÕêÔà«"?Î9íwYo?¦dƒ7W…¿àÏûÀÖ…¿æ¨Zý|˜¿ïûC½Äò
AGNbcuMG2 J075139+2657?ïÞÙuÜÞ?h.tµô?XÇ\tG?c^àå iL?dÂÿ®gØ?U[{=ó\'?ïµôC¼ËÖ?~ÈÙù]0?\Ô€ž>¦?bûÚ&µ ?}åhñ¤Q<?wiJ²™?ïqFŒ+qô?©Óÿ>4©?q:ï.v¯?sò>´6L?‹å\cù½?y3üU:?ïXjtèà)?jªV»§/?sf¡"?S9ž'b
‡?,òˆem?g|j¿¨€I?iù=™?v±)lîò?höÞ­Å­?pö2ꕌþ?tûZ³¸?e²É]¯ó?ï*¹‰Š$?•õinƖ¯?sAUÄÝ\?€&T½'?•ØŠuXT|?'
V³HŸà?ï|íÖ ¢?Š'ĵžT?uJ;R³v{?vSþbό?—½Óo/6?†}ù½âl?îeíïI?ˆžöf(qò?€
Íۄw?jvóœX\?¥¬
³ž‡Ó?‡h
üAGN4FGL J0752.2+3313?ÕÝ]Y³‹Ä@:lʁ˜ñÔÀ8÷tü+_)À<O²ÅºŠ@ùãÏrÄn@xô›Gïƒ?§-€Ä$v?¾}p@é@ˆIDíoÛ@ |ò–?¬9¥=;ʱ¿â?"À´W¿æFñ¡B…a¿æ"ύd¿ì@9
ãˆÑ¿å›«–òAGNfsrqOI 380?ïÀg=âö?s/?û\G?kq)õZ'C?d³ÞÏ»·ú?rC7pYq?g°'N,h~?ïàÒþ•Û?l¡‰Á©?DK'ÛYWU?SÈ`(3?j7oË€?gmm*K?ï`Ï6¦?Ú7ÆFˆ?v9ëå"œ?}ί›þ"–?Œ¿–HûH@?‹ºrPV9?ïþ£$´?"b:®]ž?I¥Zþ©>ï€ßC}T?!½yψ?Å@©fMN?ïoç^s}Ñ?‹§ˆT(Êo?tÖ{‰"§ï?p¯‰mŒ?‰šê¬¥°?‡ëXNÜ!?ﳬJ¸é?Š׉¶š?UHXÝ/|5?h˜n‹Jå?€kðT?ˆ–Jq0"?îòÛ‰Gx?™ë'W,—?wº–G_O?€Uz4i^&?›µùx[Ä<?–9Ÿço?ïü‡öŒ—[?.ª?¸¶m?'1\9õ?	ŸƒDH±3?6›þÃbz	?+ZÁÙç«AGN4FGL J0752.3-1631¿áÜ©†*@«Oag#%À9ÕVÅßrÂÀ< szK@ #@vè•?þ&ƒøG¥?¼ºD^ÿ"Ë?Á̈ĵ&=@ucߣi&?ú"®LˆÅ?ï…þ|rAf?äl{‰
Z\¿Ú,̼±¡£¿Õ»m߁…Q¿æÎ[}Õ¿×*Šbo
ûAGNbcu3FGL J0752.6-1629NVSS J075223-163340?îsXùQ¡?]"Â&h?tF€~}Ñí?gþSÕ¯'\?¬oúcå«?œ'B®Þ÷³?ÚßÍ×a?ÄøÄÄHL?½ª{5¢Æ‹?µ>Ì»ùy?ݵ"[x1ü?Âbµ»Òî>?허ú²Z¨?–^«E¹S»?Š>ì"5ê?ƒ>fROo2?¯÷µ0]qÉ?"Û¦p(?ç™*³2?ždºÛ+áå?¾._¤U_X?•ÆŸ%
ša?"³¹*ƒŒ?"Ùá³8Ò?êƪ°‡
»?°³GЍÇ?˜à¤†aÍ]?'4Æ?ÁÉ@®Ïih?¯—OðÀà?ÌC3pð­ý?ÂPIå?Âk›"€WÔ?¿:¾|/¯?äTLB£¾Œ?ľë&˜à?êŠIUŕ‡?¥}P¡xÎ,?šª‰ÓiNA?à_K¡w?‰lû«Ý?£Q'ÊÆ¡à?à­Ëk_Ù?ªCéíL§¬?Ê®/^ëY?©ƒ…¾³i?ÑMQ§'€¡?¦ë+¤*MIXED4FGL J0753.0+5353?å˜T&%j@>8Go*ZÀ9
Ó	ý¯ÄÀ<:wÓv4:@åø˃K¤@±Èd?¥*.B؏?©× –V!@ÕY;¸Ì@o¥åW]4?í¿ÂWþė¿Ü³_=}9¿â¶2÷¤ì¿ß‡¼Aº4š¿æ¸¸
"'r¿â}i[
AGNbll3FGL J0753.1+53534C +54.15?ïˆç¶ω?€Ðowé¼ä?a-4=Œ¹õ?T!'y?‰zÅs01?~­Æ2Y?ï—5*$?¡ê`X«Ï?…€IÈh<"?"m…Tî7ä?"Œô}gu4?"ÀŽw'ã¼?îåYE8Þ?•äpâ©"?pDp'×Ù?u
C!šŠ?ŸC»9Ô€?•HÙÈË?î ·c6¹®?'ÇZLE¶•?œ+÷Ë@?<?~N_
³×?z7˜az?k†JDbS´?îʏNÐ.?—0+'>ýú?u{¾¼ç›?hš>ñ¢? §—ð2hÄ?•'n0"…N?í«=´2Ï?µD³Q¨Hœ?™ó3K°Ò?¬/~ƒú²?¨R‹/vú®?¦kôÄÞLï?í³«g'"–?£¨§Ä´m?{ÑÙ&!|Ò?{v8ìX?°¥‡0òÁ?¢Ë†‹%á²?ì¿ÀÙ4ËJ?`¦~œw¡?±'s…î?—bÝ>
Üæ?¡´·‰"?"èª
†ÜAGN4FGL J0753.9+0923¿áTyîՆ@2g,®À:Õ±°ç"À<ZzyBáý@½sO­è0@¶¾`"‡?ÈïèÛ¡&?Ô¼K?™s@>¼ž_ç@h	S»¿?ïýCÂÍoŠ¿â'‰¢€õ¿âzSƒ4Ó¿åùP¹Uø¿ïÿþÐñ?í–Ö;
˜	AGNbcuTXS 0751+095?ïµ6¿s?|)dm‰æ‰?rܤá—NW?q'±·SY?rˆOK@þ?o§bÖ¦û?ï*&)_tÛ?˜'oí‰ìå?3sw\'?‡‡{*6Ã?'!J'uh?;w¥S@?îÿ"Év?›éŽJä1?™µ)ã–Ld?'I³Ç%£?¢ÕqÕèüÅ?"Ë´Èí'?ïS2>c	‡?tɊa¾?tӋ]	Ô?Y[^éLÖ?dÕT¡;%?rP5þŽÃ¬?ï€ÆTkDÐ?ƒ>éYQS?6q'G҆?zod"/Ρ?}/òžÞöó?uª›zguÀ?íçL¸Èçn?±ˆi"ÉҞ?–»¶ð"œ?¤ÎG4…?¦~֙±Ö?£WÔ-·®?í*¬
åpÞ?¢ˆ+†aE¥?¡Ÿ2ƒâ'?–ó0sA>"?«¶šVÓ­?œhL:XOÿ?ìåï'ÁÛz?›Æ/NÍ ?—-b ?''ñ˲
?³=!`²N?™gôúÌAGN4FGL J0754.0+0451¿àáöj*R@0$ã—­À:|­""aTÀ<~Ç¡é@ÔÈÜÓ*4?ü(æÞÆÊT?Ææ¾ûÓËo?Ç­œZêo@Wþßn@RbÊÐs?ïà&±D±
¿ÑiòâáH¿Õ'-ks¡¿Ñ´Î¾¿mê¿áarŒÖ¿æêB^IasAGNbcuGB6 J0754+0452?ï¤ÍŽWŠð?€[¶]?\ÜúæØ
?VZÔp²Ö?ƒ0ýÙw?|
É4ólì?>*C\?¾',Уˆ?[ñí`E°þ?`ìëEö¾À?ƒš2½_Ñ?~|#îéú?ïpS7"Û?}øqƒ^?dcÎsMz?c.ÕNPC?ŽæY"́Ð?{†Š4­ò?îþ4‰Ÿ|?opÍæú_?v»$[3©?R?ә^z#?šðMma¦?lcÜËSð'?ïrφ̞?†mµ5™o?hÃNü–ÙÁ?`à˜Sk?J"‰û?ƒ¾«ÖÃÕ²?îõšpÉ? ¯k[üQ¶?rt¡¥r9?{ÛW"ƹ?œÂu‰X©›?T–³ŸÏö?îó,b^™é?ŒÂvÂfí?o¿Óioíe?lA‹þ?¢y=ãÎ7?ŠíŠ÷.9?ír•ô›?ˆZ<Ñ0xˆ?‡GznÚHù?mj;©jšB?±'a|z?†¯Ñ0¸[AGN4FGL J0754.4-1148¿ÀôÂÓ,jö@ w9°$öZÀ8À"Ú›§À;­c¤G@êìž#l@?¶~¬®I?¥â‡ÁwP'?¶×ÉU"@ÅÐãe–@	û?ˆ??ãÕ6":¿×æÎÁ¹Š¿ãR­·]Ï¿¿á¡'bD˜¶¿àkö"o³í¿ìGÊϜŠæAGNbll3FGL J0754.4-1148TXS 0752-116?ïH?RŒ{	?¦¥µvbë"?`åT:@K?u*®?"ÛuEÍË?¤
¡Â5?ísÅb*?´‰ÃOÚæ?'ŸcU?"Ã7¾+v?²pd²î:—?²ì¤{Çb?ïGiŸg/?‹
î7Ùõ¥?rC±›œÚ?y¨(ä¶ßŒ?'ß£1?†¼P"K?íñæªCŠï?'ùð…p?±_
J¤?i¿TŸ*±f?¨Ú<¨ÑÀ?
*ă`ö?íŒV¢E‡?§yRÁà?oݙK9_?ic»Öû7æ?²ž^&žFÊ?¦*L*³¯?êÖ(º¨?‰ó*ÑÝ?'ªc¶ö±)? õ[û?Âr ƒ?ÀÿÃY±w1?î¤Ç¶žžL?—¹~~o£z?ƒc®òb†?"²vך'«?¡R«¨Í¯š?"IðxžX?ëy½[É2?—Éöñîf?¡—WLך?"ý·1ý?»f‡wÇÑ?–‹¼ìlëµAGN4FGL J0754.7+4823?㩔¥'ʺ@>%–À8þáv§ý
À;æêð¤Bj@ào
¤É£?ÿ¸lrïá¥?§Ÿ!Ìa ?¶	8ãÌB¹@Ûwb7,½@P°ò{³¿áM¶ígw¿Ý;$-ܲ¿áQ"'›¿ßbÓ^â8š¿ç—'¾
è¿ç½w>û¾RAGNbll3FGL J0754.8+4824GB1 0751+485?ïöb˄ÖÈ??TÁÙW?4Q#˜Sw?%>·/˜P?LLA2Û°Ê?8òÌvÂøƒ?ïÊ}ғ¶+?s	¤änÍ?Rª4²¿Nm?[残›æ?v‰}Æk?n¸p×Q?ﺤ_ßþG?u¥L^âf?`|©žÊ[?dI¯'Y?zo{?;×(?sýøÏA?ïÁñcö?Xí˜Ä¼mé?[2ÊQ DË?>%é,È"?x©ÔœœOÏ?Uå¶5Û&?ïð¶Ê4Ÿ¢?OP¨P0 •?9€û]êD?/ߺùXK'?X2,³tY—?Jè"ð׿é?ïn zQˆf?ŒÂÄü—íQ?c¿¢†–÷?l7¡Åøž=?°1K—?Šfø
&ð;?Àë©?{×ø>0?j'ÇÒpâ?t?™bÝò?¥'ýG"?s-ËÆo?ïv
fhó<?t¬ÏFó±?m"íµ?Vj1M0/?‹: Ïh¿y?rÓÛYìAGN4FGL J0756.3-6431?æüً]QüÀ1¼¡œZÀ:֞©£ÒØÀ< ö¼Š@ Š›QT±]@´¨+-?Çù¸¢ž?;1%ß/?»hø=¾Ò@€?Œ‡ã9?ï•[¬£7¿æe"®£¿Ìw3=D.-¿ãE=¼h|¿àgAøÈÔ¿ÓK‡½ÏAGNbll3FGL J0756.3-6433SUMSS J075625-643031?ïÆ!ñÜ­?‹f.‹˜Iï?DÑq¼µSù?N
ª?/Á3?zTØ÷ïú?‰™"<|?ï»ÉŠ«±?zص)=I5?Qb(`;¿ø?VšÙae²?}°~4{Ä?w–"ªCœÍ?ïe–€Æ ?µù
hDÕ?`"þfìè?aödèŽQ˜?'HÐ-žV"?PWԥд?ï2bºy&÷?uUàn)¨??eWÒø©€2?GÝXÜkm³?—®M¦i?u¿qÒx°Ý?ï˜iü¦ŒÐ?ƒ¨äÉñ`¸?UÇUFO?N±Ù=L@Ù?‡,w1«B?'_HÜÝüù?ï/~U?•aN€iè?c7º™}ñÇ?m\5Y)ò*?—¸øè0@ë?"Çšãåzë?î×Ðæ%Ó?"|Œ'"?d—ôæ·Ô?`içۊ—?¡6È 1^?W$¹y²?í•nñÇ¥h?'ÒÙWª?zʧ˜ß¯-?fÜÜ
ÁÄ?±§Ýø­Ì
?'¢?&&GAGN4FGL J0757.1-3729¿ÑJU÷áÖþÀß}úâ~À:­"àòôÀ< F.¸z/@"æìސ?ûV¯TÊ?Íá c6?ȄiF?ªe?ü¯©öÞï@ìIŸSÃ?âSˆ¾*´¿ïÆ~ŸBP?ïÿú÷''ý¿ÙiÉ<Ÿm™¿×c(ƒ×»h¿Û`~oòAGNbllNVSS J075714-372734?æÒ³Õk=!?Ê.Œ…^ú?k"ÎJÌ
'?dša'¶Z?Ò$R·ªH5?Ê3†E?æèæUV?Åkæ÷?rv%'7֛?wsP¾	>±?ӝí˜Á¤È?Å?!t*0?ë°Ãoõ?§·ðý‰?ryŽE*g?m'ÒÀ7¶?À©%Ñ~jó?§Öv6¥?ìM¼‡v¾?˜o4#ËÞ?e	–5oÑ?UvÙ#'ï@?¼åžæñ¢U?˜`À!R<?ârπäÊx?ÇUFMÂ*²?tëűˆ¢H?m3Lᗣ?ÚƱçæ{?ÇZŒ±‡T¦?Üôr®_6?Æ~kB¼X?qÜ®ðÚz`?€üs'º?áb
KmÐ?Æ`dd³ä?æº4áM?´²R"}?UÄ»Wð²?t.'˜+K?ÓkÝq"HÐ?´Œ® M#0?æÝu«Ëâ?°ŠÛN'/?s³n
Æ€?pB»ÉÅ?ÑöFð̨²?°—‰·uãâMIXED4FGL J0757.1+0956¿åÅ&³#Q@3Ø{V¸À8¾Ø»™À;ëùŒHx@
Òw[¬#@ý¶ÿÛíÒ?¤™,v«®?£Ï@ ?þçp6ÉÀ©@"®%lÌ¿ÄÙn[Ra!¿ß$ÑÜFw¿ã<æÀ"Ùf¿â¥ôñ¯e¿åC5ªøh¿Öß³#®ZòAGNbll3FGL J0757.0+0956PKS 0754+100?ïÊ\S#NË?¬NÏ? ?PÃà#õˆB?ƒÑŒÛJ?v ÞWœÈ›?§Z|^†"O?ï¨C5èLä?"R£ãðd?d[K%íd?p+&w8Ë?€Ø_Ás_Ä?~ÜÐ6Iú0?ïŸÝ7þôè?'Xnꎸ?_q™[ï\Ÿ?j3tdÁv´?"~ÈLv?€XIº(›X?ï[FR
®?p¨‰þôJÁ?yÎ"fœ?Xu"aH}?ŒSBî:?iUg>X?ïÃwðÁ7‡?v0j™bzf?Mµ½Ç"M?CBu?M?zOÜ#¾^?tƒIâ¤Ç?ïjÃ>L?¡`3?uºá&¸?‹*X~Ø^?˜""gr¥Æ?™ëŸ/a•½?ïLpÎõ ?çO+¢ ?dݯ{?fæH¬ë¨ª?"ïªfSB´?Ž-'¦C=?îdlpì|@?Ž–À\/å?~îà'h#?wïä9ßú?¡yÁ'®Õó?†§´×'
¥AGN4FGL J0758.1+1134¿êë¸ö+@@3ú\å´$_À:ŸÒ¡"$À<}၏·™@ˆßµ\Ã¥@úz¡'¶?Àñ'êRï'?¥B#ªÃÒ?å†Å&6@#¹˜'‰?›v«Ô¿äQ›2öÍQ¿ç7"+#¿ÜWGd˜…ó¿æ¨î#;n¿âLÜõ)AGNfsrq3FGL J0758.1+1130TXS 0755+117?ï×ýßážã?atˆÞK}i?MæÓÙJ?86Ûh3¶g?pD5'¸«?_¬3iTÓz?ïȕ8ÈË?sæT©–º?OÖ.CÖ?WƒòJÛ$?wÁ¨ÑÏÑÉ?p=	~al?ïšØý÷Uü?q.Õr2Ð?[Æ×é)/"?T²y
)ؚ?…Ðå‡Å?op³–Ï˔?¡û#?_h(Þõ‡?b»jÿAÏ?>ù®s=?"ðýñô¡?]Ðز?ï¬Å.â…`?u¿IŽŒÈÂ?[ËK½Í'R?Iü+ûµ?UJÄN@?tLæè Ë?ïpܖ:áË?‰Šë£I:?`Hœ"6,K?gEÖW|Š?¶³T"=?‡Š¶¬îÿ?ï<Ÿ M¢?'g©æý}T?hËûg|'y?^àŠîõ?•RŒ¦îÅ?€ÛácAù·?îÁÎzˆ¢?=4[ÙÇë?|ã#vŠÊl?`5‹;€´C? F³æÉc'?}•,&ÿ:AGN4FGL J0758.7+3746?ì?¡3Òüx@<áµ ÝDÀ;+"7ÉÀ<³bØ<l˜@\lû+@èy=Ùc?ÏBH¤ßrí?´~<Pé'?å÷SSd+#?ýœ"Áéð¿ï,æ}wúã?ï¬{­¿ÑPÜÚ¿Ö!yÍKwο꫇½Ï¿ÅoU®2XAGNrdg3FGL J0758.7+3747NGC 2484?ïÓ"?{*ÄmÞ ?`Ԅšb¦?QÀ·Éè`?"V¹¥Ø¶?xÆ/ûùf°?ïÉZ·†""?yv¤zßÌ?RÊ°~ì¦Ó?[§··5d§?vŸø&™|%?t™w^&?ï,¨'äQV?ˆèCJõ ?vå\'æ8?w£ä\q¬&?"±–‡ã±?"0¢¤û
™?ïu¾o‡?h³Íbw+?w‹±ƒH´?WéwñßÆò?†Ê¹Çî]ð?b™i¡þ1?ï%×8‹?»Ð|å?r(=ì¿[?f<£F±Q?–Óõ—
¦›?X?G˜¹Ø?ïW'c?'ÛýD=J?hÞP·¬½?rr†'NIV?'òCÓ	>ý?Ž^†¦«X'?î‹pKµ?"£L⇊?D!Ï©è?á-
ú?¢÷ò݆,?'7iC}'¯?îÔG­
1)?"uðõ±?"¾"¤·?q"ù§Æ?›U?º?€Á[•(!AGN4FGL J0758.9+2703?ìÚépœ@9ðr° ĜÀ9òÛª¶"À<mžƒä%¯@R­²«8}@Òáüߺ?¶'›}>o?ª°CÃèçN?ñï
D& ~@yıJe¿Ýpä+Ž#¿àJ¾ëÔ¿ãÑ.[]¿Ýó‹=
w}¿å'6É?¿è7fhê¥%AGNbll3FGL J0758.9+2705SDSS J075846.99+270515.5?ïØwEºQÿ?\.Ó<Ôwá?PI ºC?>RÅ"^í?od*2>Òµ?XßÀÿý?ïÉÅ^¡ÿw?wjÈÐݶQ?U42%…åL?^ž¼¼/?uÐDÀÓ ?q'æš$@?ï"\L[‰?u›'y›ÁJ?iW–Α?nÉpºèʵ?ˆ¤¼d'?mæodT§?ï'(?µ?f^Énf?vóõº'œª?Ucz}2ÿ?";!¶Øs?`aŸÜ™"x?ï²ð—(ê?o¦	o
Œ?aÈaõ갔?PkŒ­XV?}£ƒ'tò˜?kÐe''Í?ïk¬Œ÷…ï?­ì6õ_"?h€$¨Îß?saaâM³?ŽôÓ»¤<}?‡ç¤&€ìP?ï¦Ey†Õ?""»Bə¶?t³}Lõ?qÕ´×´Ç?˜~oq§ã?€ÀA•ªÙ?îÐ(ö³?™šØÍ?Œ7ÝP£g–?pà}0:Ûø?—Þòƒ™×?yjMƒòåzAGN4FGL J0759.6+1321?âü-["¡@5dàTiÀ:l¸ÿÀ<eä«æ£8@!K€0¼á?ú™C¬Äð?Åޒ\ŽvP?»«w¯?÷)sçXiN@®¡úçr?ï'h@Žf¿î˜›Ø8:Ú?ä^C¯'9¿ÝʢԀ˿Ãn9ÙënN¿äyT¼AGNbllSDSS J075936.13+132117.8?­âÚ?ˆäc%JÚ?DÀ®Ç™0?9þÑgk‹@?‰?&3'?ˆ[tgRl?ïÄέ'b?|:rPK?M«"L.B?W³w2[ÝÏ?yã8­É6ø?xļ¤Bÿ?î­¬Nä$é?˜
Õ8‰½?Q	)y"ú?@PA½o?¤œñħ/?˜,¿Ñ'®?ïGI¶éqÚ?uےcu•`?Oò'½¶–t?=îø®†åÍ?–5œòð?uO'åOw?îí4Ù?›ôûG½—?WG‹ð¼­?OµÚzYíB? t"ŒÐ–?›qŸÄD׺?ïnÚ¨¤ñ´?'W"€Cöê?[s³éú&?f†Ž¿ò¥?moº»á?ÐdÀÒ?ì­°í¸@?ªæ Âى?YÇeè?X±¼³t–?º+jx*j?ªãü}	X(?î"ßmÞ?"(Þñ?^¿" ?T•¹T¹¯?­ÐµbîyÕ?'ïä/é|AGN4FGL J0800.3+5611¿É?'țå¤@?³df±æÀ;:V=#wÀ<ÐÍ;‡•‹@ ­%èqï?þJå†×õö?Çy €"?Áþ"ÅõB?øÛkEÉ7í@;‹Œ:¶_?ï¬)¿*å¿Ø±ÁQ™{¿çýÀTïEž?î"ó—'Ø¿å€ê«Ú便åŒXž&ÇAGNbcu1RXS J080017.3+561116?ïãÏ´Cû?XoT·=t¥?A–E(˜ì?4¶t'/´?gʺ}±²ó?UÅia¼Š?ï¿ÃŒ²*Š?uœFóq?S¢ïó?X­âÞÕa?{ZÕ(Ӗ?q|¬1è?ï…ææËÈã?uBtOxZO?]cËÏ?U`ªRú™?Šã¥¬Ly«?tsùGl?ïXæú±®?pB`špk?z°{¯5#¯?_x8ïâZæ?Œn'…D½?j£bênA?ïÐ}}H
?dÏkWMÙý?NÒ1/?C~)ºbœ?s眉kU?cÎ8'§Â?ïQÙQž
ö?ۄÏ?eš˜êH]?oŽ»Æ{3?"'Ï̳,?ŠóJ¾SÞ?ï'—,Æ¡S?úŒ²€È?gâqäô?aQ{ÈK?˜*7íõ>ð?€æl-Cb?íûÉûiËÔ?çxÃDÀ?"‹Yé?'?ƒC†J°õû?¥ý³WWk&?Š%,N+uéAGN4FGL J0800.4-2257¿ç–ÿ¾ð@
戢ÑPÀÀ:L1ž½dÀ<S±Wü@@*°,Øü@…/‡­?ōi(dM?ÙÁZ]™Ž1@w¡øì@`[ÁqÏÑ?æŽMÀÓm?ÀÂQÔÒ*¿äé¾4ù‡¿åîoês¦Á¿ïÿñ7n+¿Ù¼®;è
›AGNbcuPMN J0800-2302?êAóèN?´¥Ë,îÞ`?³Ù¤Yb³?ªx´¾*v
?ºÖ‡ùÁß?«‡3m÷?ådÝÕ«?ȅƒòS?°Ô£ö	?°ÏI¢uG?ѵ]€Ÿß?ÄYðË.½?琕qѐ?°n•r¹'?Á ¯±ø¤Ü?¨ñ"U­ž™?ÀœùÖSh?¦F§?ì }7}®?~☗å/?ª*ë]~Û?ƒÈ†\Ÿ?±æ •Æ­!?ˆüND±ŠÒ?擳±Gá?¾gkù<0L?Àø » þ?µ¥ÄqÊ͸?Å 8š%Z­?´½Šÿ©Â&?Ûc"0QŠ?Í¥ö¶Í~p?¼|eðärö?½'Î7AF?Ý}SSuY/?Ë_v'Ùa?䱙С½?³ :>1—f?Æܛl,£ø?®_…—œ#?Æ\ýQNý?¬« Pn¸?å#Y–Íê?¦'ŽÂ¸è8?ª/5o? ñÐÞÁ?ÈÈjr9®M? ÁB,¯½FMIXED4FGL J0800.9+4401?ï"צ֪,@>‰ˆÁÛCÀ:Y:ßÏÞÐÀ<ŸOœ†@'ä¦èb@\ºÞ¿q?ÀuF©Éô?ÁGwÖø@1œZ>:@
åÜæuje¿ë¾«Â0O¿À*lD̹¿â¼,5èð¿â$!È`¿åeˆ…ug¿êœÞ|w AGNbll3FGL J0800.9+4401B3 0757+441?ïúv
?ÁX?5 	(»ü#?0"Ë&ü@O?(˜ygVÇ©?<,â+ý?,‰Ô1ʹ?ïâ¼lq1?lnþ«æ$?Aî¾Þª?M@F…´‹?hÁÂWPè\?fõPa‡Óu?ï˟?bɛ=S_³?Qµ!Ï(?Tïï"ç[?uÃ8NÓ<?]ñ¸‹ð?ïà.âÒ®Ê?J
`z‡/?R…l½n?1ôþár?fŽgMÍVu?Fî­¥p¹?ïô<¾Þ]Õ?H·'†ò?F«>›o²?@-㆜³	?HaÆÑqûË?=P$º–ó=?悔'r3?'2:Æjª
?Rþßnçö"?akžy"?ƒ›ô±¥üj?€#Á_?ï­,îömZ?q(ž§nó?Y2á-öÁ?X'v4›°N?Žh­³U?m—ž'*6?ï²D	^r?fÉ{›ô]?dü›ß~‡?MyÂÄJD?|_­iwe?c›Øë>~øAGN4FGL J0801.1+1335?äeˆžÅ[@5yj&åGÀ;UDêÜ0À<˜'6ôˆÓ@GCeÛQ@oå]½Jy?Ï_×@™"P?®3‰ð.PË?â{wN:@M€VQ›S?êم!½j?à-‰Àނ¿ì\Þþ'¹¿¾_g¥«¡¿év±'n"ÿïÿûbâMhAGNbllNVSS J080115+133643?ïxûï¥ö?'î3SYc]?cˆ—p"l?Yæø»žÂD?ŒÞÞQ—gß?ŠÝG{
)?Ie$?˜8›¸P?]rC^
?bÇX ~Zç?ƒœo§ú¥¹?~`Ûª8·Ò?îðʯù¤?ŽÎAó9?v_þÖÔÊ]?výÉû©]?œNªY›¬ã?Œ7O‰R?ï~	xØ7?{Ҟ§,J¨?ƒi5Þg3«?i­ô[8`F?•{£ÙFTd?w</XÐ?ïï5·Ù?'a\€"hú?t¶%Aá't?ltz:Uª?˜Ô"Ðèø?òùf›°ï?ïoãùËD?˜é§òúhN?r*I™m?ŽmàfU?šq6Ä¥E?•ïØ÷o¼?î*/*(â;?—ß´7û?€á–¡E?|I}Œo§ê?©$­yï[ø?–Lªð²nÍ?í]é{jj¾?•ÍÁÞ?œ?™6`O¦$z?ˆ¨91´^ë?­†8$õÝÜ?'¬aK§ýAGN4FGL J0801.1+6444?ç¼K@¬SÂ@?¿#FV%§À:ܯæ8óÀ<ͼª R@ïÛ›l@^	Zõ?ÀQמ?Ž_^E–ÉA?Ð(€ý–nA@±ýx¼)g?Òdè'4ù¿å|, oa7¿ä& Z¾h¿Ú•ï ·E&¿á?›÷Aë]¿àLÜ¢,æAGNbllRX J0801.0+6444?ïøMÇ3/Ø?aVû ´‹Ñ?+sÕÑ*½*?:Ê×\ôt?Gëîoûh†?\!Ó†"÷?ïäö@RoR?n—v'õ:ö?:–­-wT?EOEÍ3O?g¶ê"v4(?k""<ŸGu?ïÄó«oH?g"º_÷\N?KU¥[4us?5ml.òDÍ?zu­{U»?fë4|kƒÚ?ïëªÀ™Ÿ?G—.ò?;yü·–'ö?°°l¿À?aßÀÞ?GÍæ'U?ïï€íl*?c¢Ô0df?>q$Cwí+?@‡æ@Äí?Yc5EñJ?`uÎjß?ï¶	à166?'Øý¸u"?IŒ`ž?äy?WEáö$–?€äÁÙÔE0?€fôÊM†¾?ïŒÎ€3ʐ?zˆÂ£ª?U­xØ»º?Ri]Ó?Š°ã»_?yªGaG~~?￱ëÂRÃ?e6)}iò"?TŽ	=Ïm?;òª{	?{‡Ñr‡]?e5PuAGN4FGL J0801.3+6631?Ê3XK_hµ@?¥yžQ?À:Ö§"þÀ<£dύqm@î8­Ež@©¸ËŽ?Ë{«r	1Ø?ɔçÙ³Ñ?öl×[œ@¨»R¦ëè?é'ôÛߏG¿â̎\X¿é¦Ê;"¿âa‹¶'¿é–lˆ¿Vÿïþí{˜ý'AGNbcuGB6 J0801+6639?ïE\ÿ=?Y˜Nu@å?{~3ž%b?xÍÐÐãî?tÓ1Wö=?‰¸øáQô?ï¨ß8V«?y+{X†s?`mƒçWÉà?_øT'Œ?àç5¬¨Ì?t&J(Úu?ï+•$iì®?†®lU÷º?n|7ó‡-?€{`er?'±¼c
º?| ¼mÃú¯?ïpU¬@ "?f{Ž§ß>?}"*|;I?V™7´¼T?…Y"ËókÅ?`TbÍ%?î.y4ãü?¡ôr"(q?'HÉَ?‰ÚBÑí»2?¤™d4"ò?nÞ2pƒ?ï3^QD?–;(Úp£?vq©íXÈ?€ö‹ÿ¯?™áOM¶L?·¡WÙ#Ö?íí­Fc€r?›óAòø;?š?áÊéPo?"éôb¦?¤:²›'¯?ŽU«x×;Â?îii^¤ŒM?ƒ!cù^Ü?"s½Ÿ¯ÉŒ?uñ‹dùÝ?Ÿ_'äÈ?{·+›¯1AGN4FGL J0802.0+1006¿ÖXÈ×Rjd@491"·ºíÀ:€®@ð‹À<zÛmy€@Ÿ*Þzõ?ÿM"þ1ɧ?Á#ÖÉÐÃý?¼)m↝?üI¬|]?ûÌpk¢æI¿î1ºÂß
A?ÖW•}«&Š¿à C=¿Û|ÂHds¿ä+"Xœ‰¿âr¼Jž‰ÃAGNbll3FGL J0802.0+1005NVSS J080159+100535?ïÁü?½@?j©íÚMÅ?Rxã%ߤŸ?B¨¼r¶?zàÉ
úʬ?hïÆ$Ô?ï>âÔԋ¼?'yôøqÔ?|ÎLäѦ?"íF1@(Š?ðŠN:/?‡¸®&H6?ïv@Xà–Ù?vìøVŠp?h™;‰Cº-?i³©Äk˜?ŒIšò—ß?p¼·KžH‡?íÅØÈO?~󩊜^m?–‡¸ÿ7 ?pû#/ƒþ?¨^—C.Ü?yÞ?ï‰vá*IL?z]=c?eq'u…S—?U¯Ø¥Ú?ˆEãM½""?wÈri»Æ?íËÝAú?«ðbʸf?'ìFk}—?›3€n¦‹?©Ì賶?¤Ên¼ŠÛ?ï¼¹ü‡ó?†F°3Q´?q—÷E*ÞN?gã\"ñÀ?š¢jðÜ?ƒ8¿Òyó)?ê"IåšÔ?–¶³àáy?©K.mé?‰)—±á/?¾¸¡ç›Û?"Éw8äAGN4FGL J0802.3-0942¿êi\\n¸@%çÄÁe~À9Ï6¿yÀ<#Ÿ¢È…@ 0ÊڄEt?ýî%\°Úÿ?¸ƒ|-""?¦Öñ`Lh[?ñ7¼šO¡ÿ@œ•.ûÁ¿ÕTúe
¿è‹Ëz½5€¿ÞßeUÅ¿Ù8I½¹3"¿ØϹü‰Ð¿æŠQýù•ƒAGNbcu3FGL J0802.3-0941WISEA J080215.63-094250.9?$W<?~Ç´ÉÈ?P¥gÂd??ۉ‹³Êt?ˆ»ÊÇÝ×?}¥Å¶%ëö?ïA{´<™J?›xR£Æ+9?Uno€µ¬Ô?avMè'à†?–y¢|mï?šƒÜMÄ?ï/ÛÀ¹ Ñ?ƒå»JNî?hEb¨P ?c±Œt——?–ûÕý6ÇÉ?'žLÀz¿q?ïl¾#?sÉ´Q›ö?e¦F¬»?EG̺ޮ¼?œ¨)ÀÞ[?s@ób}@¥?îò¦÷·B]?"/Œ2ôa ?fd]CÈAÑ?Z's¨?žÞ•_Ù"?"-Ô8K×â?îMTœmF?°©ìdºL?eíÿFüy?v ÚýNaB?©ËÖCU?°¿Å¦ˆ'?T÷(?™×œ^šêý?wO§)ôsñ?rö~í0ó?«»°Ù¸ú?˜}J!öÆ?í\'mN¯]?Ž‹¿	—bÆ?{˜m±s©ë?d2°¬?³e=ºì<¹?×ØÓóAGN4FGL J0803.0+2439¿çŽ'iä!@:»'ˆÛÀ;o"1zÌÀ<ºëªÞe|@ á:á}]ú@¢(ÁÀ)P?ÂX\›D¿¶YXê?ð·…Ýúòz@ýµ\Í¿":B¤â1¿âùóv"Á›¿äï:€.Ž‰¿í
DVq%Ý?܌%þpÛ¿Á
ôeB$AGNbllNVSS J080307+243749?ï	 Ù²l?·2¾ðËl–?g~÷6?"ßìÒ5?›íyþdB¡?·	Ó/œ¹?ï00‰W# ?¤,ûª"?ptU%Å?x^ÆÇ«?•øÑÆ-a½?¢kIÚQ‹1?îÛWCD	?'}"²y0æ?jˋ¤!~ž?rîª<
L? ¢áÐkÈ
?'ñž¢XS?ï²"+ü¼?qžÝÚþ?+œ(Hš?%Íq±»@M?ƒ.Z‹-Ç?q£ÙÄÛ?í™%x_.?ºØàì¿[u?nT°'nÜ
?s~Åô??²D.¶<`°?ºyǵ>nX?2`5±?­")Úö¯j?q7ٌT?ƒ§µ³ t?¤PÜÞµ$?«yå•	?îDælŽ§?—ÿÖLmåã?t¾}š?wmü!Äû?¬áé—óL?—"#']=¦?îvk›sRL?•®ã¨'x?Qç2–Ï"?Rǐ î½Û?¨
íÂ?•¯:'ÂC…AGN4FGL J0803.2-0337?r_!K@,b€àe0À9<IðuÀ<3{W3@=ÚÞ]mï?ÿ×¾³.–?ªu¾É?—Hº²™?æ—VO—î@	íÄoÜû¿³ÂA-œÆJ¿Ý!4ƒqý¿áwÂ^´Á=¿ÞæNþë­ã¿æÑE7Aµ­?•lÖÂïÔ9AGNfsrq3FGL J0803.3-0339TXS 0800-034?ïäVŠ%]?`cæ}y²±?8yÁ¸ç?*ÏîßouÍ?háqvD<á?^¾²æSå?ïь2ÓM?xS»HRðŒ?QCǐ"ë_?]e…aô|Â?ré¡ašh?sk¬í?ï éUÞG¸?|GʑUŸ¼?^ý$³6?g݃¦<?ƒæ&Ï#?yúž<y¬Œ?ïŸwÌë*±?cÆނIl?bU/Ñ6»i?Bæ^ñŽ<?ƒŒÀܖPß?`ä&ЍBg?︞Ì_P?x¢;˜ú?M¡a0·+?C±$øø?üĤG?vyþàürÂ?ï|ÒP;Ï?§,?Г?\¨AÇì?k߸2Él?6cÜv͍?Á$"q?ïZ×9bLP?‡N¿Ç?fžS 94˜?l©½?'ÑNoWYa?"ÞüÂaMž?ï•rî_?£hgÙì8?vF7y©8?^Öâœ
@Ú?—{Ñ
¢u£?z{ŸÑ€¶AGN4FGL J0803.5+2046?ïZV9adc@8ÉDg8~À;9Òïü|¾À<¬@ä@)°-ï#?ÿüS"¾?×7¤¨§ÿ?襢¡€è@	/ËOKE@
³Ë'åö??ïüÕ,ß¿­%ëbd#¿ä'§C¦Gþ¿ïÝu@ô¼Ö¿ïýè-{cN?ïpÿь$AGNbcuGB6 B0800+2046?ï¡ÉØÜ?ˆô ÁÐ@?TQåÕÙ?UHj(È?…™'¶·?‡¨5`+†8?îӇC_¯? òRcW?Ž×@¨˜ŽL?"Îp¿DsÙ?–#oÁõ?À¬ðóÏn?í¹R>Å?¢Qü³Ÿ?˜Óu-_¦Ý?'=ü²:Ò?±­X$o¦?žÝ¾
?ïE:Ł\•?xœ(¥E¶L?€±oifkZ?i›`ññ"?ÿß<ɱ{?rËü¹z•?ï,»Iî?"®àáSWñ?[Ú?®ñ?^ܬG?Œ½´ÀŒX±?'ýN8¶ï…?ì¼8½"?¹W—€¢˜??¥§.Â0Æ?°M
ô¢c?®˜Á>Œï?«÷Eù‹?ë¿ÒvìÖ?¨ –'f?¡çÒ lÌ?•×dÃ]".?¹
'ú!Âé?£˜€–£°?íàÎ@.21?™_P½âI?'Ž'Y­f?…"Ý?£¾h?©+ÓRÙÞÝ?•7hnuËÖAGN4FGL J0804.0-3629¿ÁC·dÛ¡ÒÀ á÷×<'À9ZÙæÃ1À;±¦Ùóü¼@ ¨%o{8?ú±À×ÌP?¹+³b¢3?Í/ö¨=vX@Ýð
¿w@{)(î5Ó¿èÁÿ)%¿Õ¶º¼©éô¿×¯[bQXã¿Ã(™|=h@¿áéñ€‹U´¿â	,«AGNbll3FGL J0804.0-3629NVSS J080405-362919?ï'
l,ׂ?{I¿ÓžYé?uDc5r;P?mpM‹E<?€Úsb¨È?rE%a´1?ê½90o«×?Á´ßg¦z?k	ŒJ?v"(
G?Ğõ
³œÐ?ÀãˆAÖ?íý'8ªŸ?œ{=dĹ?˜'€!£hÐ?'zý
ýëñ?¤,gc?"ÖWõf?ì~ñ-üÒ?'V›fO´?ƒ"`·Ù«?eƒHs[?¹¦2La
:?']'ëûG?ï1—bîÉ?'"B¨Ì0}?ƒ}ևC%N?|p{F<?":áÎË@?‹‹#o¬ò?ã")uŗ?ËèÐâ2?xº‰v\bâ?‡‡¡ƒúŸ9?ÙXÂï~R–?˒‹_Ãé?ëýÛÚJ¨Š?©g«0[?­¾FÏ¡?¡a'#Žú?±ˆBÇb? ŽÅ½$h^?ç³kž£]?§k…®,?–À¢SÚ+?ƒã'"ðR-?ÎZ=:jv?¦6'
@Q¨AGN4FGL J0804.5+0414¿æV>&ÆE@2.úÆ\À:a(	4À<U°i@íÊt­Ñà@œn`/ë€?¼q{BkŠh?¸LmbÁ?øNI¿f²½@
bK¤™'?ïýêa2Iÿ¿ãŒnØû¯8¿çÎÛ/f¿æú¤¬S¿èX<8d¿ïÿÈl뻥AGNbcu3FGL J0804.4+0418TXS 0802+043?ïw 1ñ=?¶oÉ	]q¬?ƒ'4Eۘ?£ÂJø'á?~!~"²-B?²÷xŽZkô?ïÀ+—?y–´T°?Y¡‰
?b¦#ñó'?y®X eÊ?s9z²:/À?ffiïÁÌò?sžz3·º?aKëÔåv?eq°F"HÏ?€Œ	
ôÎ?o#JtMÈË?ïVì~w?cPж¾þæ?rPä®qÁ.?Pd"äïL?'Ñwã°£Õ?_Qô6™ªA?ﮨøÑÍ?­´e'%~?i@*Ö+	?zºó;È\?|nG'1à?­›°|ƒ?ï?~þì7T?˜³'^ÔÜ?píúŠ{?Œ¦r™EM÷?"ÔÞèMôº?'æWg›?ïi‰¡Ýh"?S"‰·ß¸?q‹ô²õVH?s@F3n
?Œ×)SÝä?{­šDFÑU?îªÌŒ¶b?"L¤)‡¼?Œ‡é»<xú?q1ùf!¶Î?œby‹ ÷K?_oL/ŸAGN4FGL J0804.9-0624?Ú÷›3û]@*Xä2DëÀ:‡ö'À<'õ»Ÿí@ ˜¢=W#}?üSd"?À©õ‡V ?½=ú·k¼'?þ;ýÝ@³6É?Ïy?Ð*ý$"®¿À
~ß06¿Æ"àå]'W¿Ü>&áì¿Ûm·_þ¿á¶óF´xAGNbcu3FGL J0805.0-06221RXS J080458.3-062432?ïŽubÊ?{Æ"C`ϼ?Us|ô"IR?D¶ÿ4ß7N?‰´7Ë5'u?z…`ë¶?ïO"]¶Š?•[V2©¯î?c
É?iXÆe¼?"™Â€ºòÒ?"JëùAB?ïÍT‡Þ?ˆ¢Hµh'–?u0i,$a?tîØ
£?˜:;QB§?"³Ñ5·§?íÔ}^ƒ!?z†8­ŠV?ƒß4;š'œ?[·Æ#'
Â?­ÇE'Q?yálòÀ?îȯƤ/?—­úcXËæ?r$>¬ð¯Ç?hßò±˜?¡0{¼Ç˜œ?•ðÍsjú®?íñÆã¬?°Íøi"?zF#?¶ýݯÖÄ?­"©³uY?®\¨¿ªº?íùv=ôØ/?™ÛyNO¸2?=¾{&?xçìÖ½ô?¬%¯ßØÍ?—'%¸
è?êñ´i9æ'?'.ö(3ýh?"µ‡C¨6Æ?uÏg¦U?ÁÂ}q"Š¢?À÷
öđAGN4FGL J0805.0+6746¿î¢«Lä#@?䖚
Ø¡À;'çv¯ŠÀ=Ò®Že@¹+x~ÁÒ?ý3o~=Á?ÔJÙã5ÄÞ?ÜדdÌ2s@dZ˜Ó@ºŠ.¾³¿ïÿ–þߙƒ?ïÿ·pD5º¿À@˜ ¯¿ä<UxØY¿ã¬(|öˤ¿ïÿõƒ¥;ŽAGNbcuGB6 J0805+6745?ïÔ×
 -?hÂûZ ?^]ÌÓ×¢?UHµ°akZ?lËB¸|'Ø?b>±˜ø4´?ï¤`Ë­ú
?'P Y?ev;šÜ¡î?m"óqº?Š><8°ð?xù9C˜Þ?îÖ"Xð\?"›?u±"þ?"oV-Âޝ?†Cûfi÷?›	Ïâ€é?àèËv"˜?ï-í'=€?uð–ó¥hU?¥.pr?c
ù,0V?'y¾»oµÎ?r…ô(ém?ï£gÏ®9Ë?x¸cæ??rŸÆ€î­?lÅL~G~{?{¬QÆàéS?pÕ©}"ëƒ?ï¦|šÊ
?˜™\9W?y]äZߪ?ƒÊ¶e`æ¢?—Kì°ÎÝ?''NšIÖ?î3¶±
?›2¾Ü-ij?
ßü$_M?Š€¬J¼µÕ?¥‹—'@T?•æTÆ{Þ?íø2ȉò?ƒ=Œ¨ou?yÅ\δš?zÓÍa8$m?¨žb+CO¶?ŽØÙö£WAGN4FGL J0805.1+7744¿ÍUžmýß@>Z<d4\ÿÀ:ƒ4-.6tÀ<{Wɼ@öFBÚp@]­Z@¾6?¹8¡ èÝ¿³éKó?÷5Ë(‡Þ†@Τ¬È"¿Ð"Ï£@âH¿âFó¤§ê•¿éçåWMÒ¿â©i»…|¬¿ê¦>"z~K¿ïõ¬EmÈAGNbcu3FGL J0807.1+7744WN B0759.6+7754?ïöC™gõ?E"zFI½È?B`ÿíeò?6ÅÕ¤'_L?Dë9sï?<g¡ƒPÝ?ïà3&H??q++Ãû\u?DTB‡Šù?VX<q¹k?j·É,q´Œ?jk§¶mZæ?ï®o˜O}Ó?{ݤ.÷¥ñ?^•(š¨?hÙw€7p?€'t߆?w"eµ×áÕ?ïêÃå"ç%?EJ]Ñøj?I®FMÓR?0úG¾r?]¡óF'÷?BÑÓÇò‹?ïîjƔÆÃ?WÏ'.eîš?W	0ð««Â?S¹bÝ#íÕ?HBƒjËΊ?BaŠ"ۗ;?ï¯]XÔ5*?Â³ÀuŸ>?O6Վ¼bì?\jÀ!'?'5<teݞ?€`eÞe­W?ïujPçà5?'˜!¯09n?iF¸y˜B?p\fyÛß÷?Œcš
TÈ?î–YžÛç?ï´:×í<Y?i¨Û×-Û$?jI¾"WžC?X"ÿ,l¯?x½´ù•Üa?dk¢ÁµAGN4FGL J0805.2-0110¿í†'ºý8ó@/"(ÂzÀ9±Ç²±˜"À<,<{±QF@W¨—ä7Í@ÉË«d9?´"D•ÜÑ?Á½…\ @çüMÃØ@ ççÛF?vRdë€Û̿ݲ´Þ¤'¿ç¡&Ö-Ÿ¿æ
ݹ.4¿êö&B4¿ïÿÿ>¹úAGNfsrq3FGL J0805.2-0112PKS B0802-010?ïÞ³´Db'?bÎôÒeÃ?M½±žc×?B9ÿ=?iÜß8½Z?`ûÕ»##?ïÝ7¼ëê[?rÑ˲A?F%·eq;?S´<u³û?m>ÕCb1?n(ÌGVÙ¾?ŽLÏ?}ÛŽ;Ð7?lfï•}ø?rb¸îåN?ƒ… •¹@?v-—µå9á?ïÝfmGV+?Mù±½Ê©£?Oê˜Rîà;?2›êc"ŽQ?jžì¼A¿\?HÇzž·>?ïŝ1dã?qŸ›ëž>-?]2MQ=Ê?U•öFϺ?uäã›ý–S?oÙqoÐ?ï˜rû?‰m<ý?['âæןk?k.$emø–?†qÖHÇP?†8ôr–?ï0 â–Á+?‰[WÕÚ¨?z_Åü»µ?zd»¢Í.Ð?"f˵!iÅ?ƒB(‹e×|?ï¤>L'1.?j±'m$êõ?eЭr,±?Qb»:˜ø?|A†Às'?eºív~AGN4FGL J0805.4+6147¿àƒŽâ¨Ï@@.}ªOÊCÀ9ºi¨:FMÀ<e(wŽ'@k`ÊÆi@$>úè?µ¶e)O…?Ǟ^ºËm|@
k4*©ø@˜‡C'&¿ÏBi‡¿å¤ÇÛØX¿ë	øÂ!¿é»©Y*=Á¿î_Jé2^!¿ïY/±žsAGNfsrq3FGL J0805.4+6144TXS 0800+618?ïÄ;;?q/?¤+ù49G?pç]R†¬¢?—.¬‰â÷™?iö
C\ïm?'—lS÷_.?ïÙÛ,zÌ?o´WÝÏåï?IÐÆìɋ?TÑ&ªäò•?o°¡ür4ƒ?h*Éâtš?ïn3IûÄ?…Ò‡]:ü?|Ñ%íêo›?€ÁÿÌûÝ?†`;U-?|«Ý¯l@z?ïö¨k¢?5G‹ú28?@ÕdX·?'¥ÿÛ2øÙ?FÏúžS'?+öê<o:?ï×¼W3Ã|?hm¥€EË<?i'LÎk?aâÿWNF?^\Lvñ?V7ÀmW°?ï—Ø$øD?ˆÒPÿ¨Àt?U:šâH?c§Çh§?‡iϏe\R?†£~6÷ñ?îêüVcu,?"`;Ò¯?{ýÂÝ?‹Aa…gD?"·/ˆ'?‡>þ/ªÄc?ïज«"?Y®Ž^U2{?\¡TúßSë?L¨gÖCnù?a;ã%Ô?N¸œÓ
AGN4FGL J0805.4+7534?é:é»èE@>Ëeºnü7À8áhSÀ;ÿ.Y°@Aé~3b?ý&ÈVE†ó?¡'ccý?™_»…iÐ?øéq-iŖ@Lœ«œÑ\¿×öÞN«¿ÕHåL"C¿ßÃcl‹ï¿ÙÏ¾ï"x¿ÛtúÓÆ;¿Þ¬Âû<ÍAGNbll3FGL J0805.4+7534RX J0805.4+7534?ïò°ôóv?aæíСm?,»=ðÍ2Á?!×ðFR?Wn¨Ct?a•mK?ïÓ{´ù"Í?r"lØc¸p?GÍâK}‡ÿ?Q$€¿5f?sHi8Ca€?pt`˜ÿ½?ï~€Ü?ãÏÐî?[Aà}·C?kÐ;:Â_h?Œ÷Àޅp"?‹z¾±õê?ï­Áí~PÆ?a&Y˜'­?bÛÜ(ò'?BàÄ>FV?ÐE´ŸÄ?\ë¾{#?ïæ\¶~?a	³DÎ?<i*Éð!s?0*2p"rö?eÕ~"Jý²?`…üßF?ïŒ"iµT?‹1Ö<Ä?WKm§Ni??b¹oL'ò'?Š
øÑ7ö?‰kx6,×?ï3˜¸•¦?"²wV»²û?]ì·ÆyÐ<?fù"¢‹•~?—®rK<?"M,E4;?ïO^<ýY?y×ÿ;¸?s½«[]Ö?\N2Z «v?'0Îedo?v!Ø/AGN4FGL J0805.8-2331¿í¦vUæ@õĊÞìÀ:ÈlÁÊ:À<GÛZ.I¿@hÝao†¡@*':ƒŽ?Ç刚î®I?²Ë.'?îꀥ+ô?ÿÑɶÂÊ¿ïÏ@À£\?ïùåi{Ĝ¿ä(íßìå¿ãûØSÍ¿à-d‡im¿é¾@_‰ÓAGNbcuNVSS J080604-233333?íkZ"¹kO?¡å rë?cçʕS|?QB!'õD?´óLýÚm? à²ÔEj'?èԛíJµu?¼ˆÙ9äõ…?€=3Û°Z?€—JôẤ?Ë©½T;?»¶ê箿?íp"¿¡&g?š
%•2N(?{Áí¨<:?s¾ñ?²¿C)ì#?˜Æ—k¦s?îä`5?ƒG:¹¨Åi?'ªîg9'£?dTwpg°?«-&k®Ž?'W¹J×?é"õ˜ñ?´ü2åtRQ?z>œîAÍd?m!«d/ô÷?Ê¢4·†ƒV?´ÏÙ¥*úÞ?àÚñ<»´?ÅæºYWµ?Žfÿ#Ù?•1tML?ÝVì¾ã2È?Åd"®?é°Bæ.¢?ª:FMÇR?ŠÉkM¾À?z›ðK®…?ǝÑ5šÊ?©?ƂÁø?êäRR2Qâ?œÂÆmé?–=¿¬?'½—œ«%?Á§Ó	Æ?š¼åדWêAGN4FGL J0805.9+3834?ï÷[ùri¡@>o|¯Ý©À:¸""œÚ—À<ª#}@ëÇ8ä"@ïáÝÖ
?À5a¶©Iæ?˜â¬/t7?ÛIÝC½o@Ð2ÕÀ;o?Òïaz¿±>Y,3s¿æüz9'Í¿×ÙÜÀ4ãâ¿ßÌ´ðã¿ë—p"½'ÆAGNbllNVSS J080551+383538?ïí`/Õ?PTq"Níå?@dÈ`6]?1R"WÄwÑ?]
=IDi'?L,d¹®ð?ïåoØÁ?jvÜDÝ?=6äE¼?G˦(ÿ%h?fé¢qâ¡ò?e‡Ï3XÃÎ?ï«áF×U?vØ«ÌýÂ?X¨ÀŠÀ	?b5Ú)*³?'"ï•ð?ruҍ&©Ã?ï×ä8="?M¯ØOFß?T"¸òøJ?3Ëéѽe?n§?P9Ë?K:‹Mwž!?ïÝí	òáÎ?`ð+q¯X?Lt¦ƒw½v??*Û*ó¦?jõÌ<²w‡?^e^"åôŸ?ï°›§Õ‹?Õ]¶²¸³?L©Zƒó;?X–ÓOѯ?'0È(/‡?€:#Àa?ïi(^T/h?'EÅAø"?d'öDò?or"ÂÖY?J±Øi]ô?ƒèI
Ñ?y"ü)?hÕ…¥FM?k"Ç‹»þ¨?S ?q¢2.?"®¯¿ñ~$?f8¸'«]AGN4FGL J0806.1-0458?ïþÞ
M+¾@,J•BCÀ;NŒ"¸'¬À<'"ØAu@mö¶@?ùéôÆ)?Ý
¦a©]?ì]d[Ø@§R°Å/@DG?"¥A?Í$‡^X¥Þ¿ïþßÙïÊÿ?ïÚ%`ÙR¿äŠÿ?:Ó¿â &`¼Ù:¿ðAGNbcuCRATES J080608.79-045411.4?éÜ.eÝÄ0?ˎ—Ôé§?Mƒ÷Š?Š‰<ôï^?Çzn)ÃÈ?Ë$E†¿CÅ?íeED‹Rã?¸@Ž,×c?'Û‡lô´˜?šMêˆcU)?°^ôýC?´3G	?êä*ö½zä?°cjx¥ËZ?¢)¿czE?›°NKnf±?¿ÉȘW½?®»'*Ïo?ì©Óù|?›¹¨Üg?…|ѵ5?tRÖ`z6M?¸͂cÎÛ?™ñ…0.…Ÿ?è=ÀZM©V?Ë®Ît—¬…?•Uwÿá6?¢3ÀÀÑ¡?Ì^O––/?Êxèg:ªT?êžÍ?ZÖ2?ĨO	R?¥)6U㝅?°ŒO¬ï~?À:}lß?Â;"ç¿R¢?é÷"á39?±SµÇ?šM@TÍÅm?•xy3S±±?ÄØDq–g­?°íÁ,¦>R?è±»TS?²-H²?‰^yWæ¹?'	©&øc?Ë£,!h|ã?±ÈÍàLwAGN4FGL J0806.5+4503?×-‡ùšFy@?«À~à°¯À:µ *­R´À<ŽIöÄ@&üª‹@ð×°´h?ÉÂõ³uã²?ÀT…h_9÷?óNcaÏ(@úŽ±´Ÿ?ïþrâÅB¿é]÷vĂ¿áJ
À2	½¿ìQµ(kY¿ïÿݛQ)¾?ïÑB*òÈAGNfsrqB3 0803+452?ïèla8e]?a—™œñ(Q?AuVÄáߗ?H+cÉd¡?c6Ib*·?^'?ÒV»*?ïÀ ¼Ÿ>?~þÆWii?WL÷ P·?cEeB*™?z)±ûH^á?xs_û•›‰?ï"¹ê"?q|Àx‰?€Ec~Uù?"¹¿?J·—?"†,¦èfÐ?‰À'«¿?ïäGpé|?Lü$¨?KlÀ*DË?4'§m?dò³¦âÂ?GØßðÛ3?ï¿üÁuða?z˛>Xö?U0;†dÅ¿?T1{È8?zµGAÒB?y^ƒ…~ê?ï[6A?•ãTØÝAÞ?f>ßrA•?xƌ¿öÑ?'Ô=:M)?'54å¿?î™}#0œ?"Ù›WØÛ®?ƒ*€Èl‰Ï?…xÛ·_øð?¡—sGÍ?'ŒIþ:}á?ï¢Íéòm?q4TËÕE2?bނÍjê?SÒßø®ëü?'"äʾ?n*€é"ÏAGN4FGL J0806.5+5930?êqûó€ë£@@Ig#$È6À:}Æp'9SÀ<«Ù§¦¢—@ ¼²MoŸ@%¥á¦x¥?·gŸïôð¿'¤üñz#?Ú}"ÛF-@£I€C‡?á¶Ì7«h¿ç}€H9Ö¿ã "IÖä¿à%°"±"¿Ç-\"H¿ègõ¢ƒøóAGNbll3FGL J0806.6+5933SBS 0802+596?ïè›öÒ@?UÚÞCPçk?ECÙ½¸?5)îÞës?b#ø."µ¢?RðXqI?ïá^uô#?m\?ä?=`'OYÉ?GpÝ
5G?jõ†Gð¤?i´Üwšk?ï¤eßq®Þ?v#p«¤·?Tk 8wqM?aCsƒ 
?"Y ¤âa?tGÒíò8!?ïÚ)ÛàTÙ?ŘÌÊ?GtRÎTg©?.žn[W?oùª{ÁÓ?RxJxûè?ïÏô5?jž,°øò?W%Å+¯¶?J_ÏD]"f?rµÆ¹¼?f¯'xÆäÎ?ï¬$î÷Äó?'<Y'†e?JßAá'w?V› Ãy"ì?ƒHÐ1eè?€¼»è ?ïK¢íD*k?"僺К?Y(Êñç?\Ú߁$ò?"ùµ[Ýp?ƒ¯…ÑR"ü?ïˆõªðÊ?r8£t3»?b)îƒ?Q
–hVŠ?‰B
ËçÈÇ?r-º	;AGN4FGL J0806.9-2151¿ã·jaÀá@fð¸»À:ÞØh'À<m¹ô'ô<@dM¢JBC@V§ý	«z?Ê0mƂý?Áw$ºŸR?÷;º‹¨â?ø<N¿ÓÀ?ïì²²$«¿épà'ÒU¿äX§–²^Œ¿Ì\!©s~¿ë~o§WÈ>¿ÑAqºWCAGNbcuTXS 0804-217?ç"Vq¯Mi?Ê©ªUK?…ùúŒ¶wÅ?ƒ9²yS?ÐGƒH·±?Éîáûï5i?å`šSAµF?ÀBG1[±p?—Ã&vZ|?"oxáý±?Ó˜ò»Úó?¿Çg»® ?í'üq¼A ?œÈÐîä\ˆ?ƒi

P?{ÃÈ)?´RúÐu‹¹?›Jٍ½}?ëèïq;n?'‡}CiåŒ?œ*h3pî?z<€‰U?¹­êg?aêð¾m?áÐXzû?ÈÊ*nq*m?'^2á	âÛ?ˆ±œÕBM?ܦ| aõ>?ÈS["Ïf?××.<JÖ_?Æ5›î2£?£­g,ºA?¥éºôQ.?âْo²,?Æ ËÛéD?éMk½,4«?«ùRÚËñŽ?:›¾T<'?…ª¸7UN?ÈÂý"ò™C?ªÕW¼?åV¸Î4£B?¥n¼—?± ¿‹mG[?™+"\eƒ?Ñ
^€òad?¤ÙWÚéb]MIXED4FGL J0807.0-6102¿ÑKØØÁ2À.¾ó'ªÀ;¤˜ÑÀ<ª^Ô¡­d@¦/ÕÔ¦?ÿÜÀ_×?Σ:Xš¡?×êÈ@ +š@F™&­ó@ŽªÙÝ×a¿ïÿý`éNä?ïÿþó…õ¿Þt—A$¸q¿Ö×=¾ýVW¿ëbÛ, Å¿ïÿöùŠpAGNbcuPMN J0806-6101?ïLmÊø?–µŽ¯À(x?ƒÞ¬Õş?Š…YóN\?‰!$|†ð<?Œ®Éô®¨?ïA>ò=!?–ÏqÆ*—?|ф=!(±?ƒPPKY1*?£À¯ %¬?!0
ö*?êàÕsˏò?¯%ÎP‹?¥ÂÄר …?›Ù5À›–?¾ñõa|®?«Þ¦¾Þ1?í×Éßä4?ƒÂ$Š"g?šËÆ9 7?usâS(ø?¥u|*‰E­?}T…S»»?îóc"XP?››â2à^?¥ú""?ˆœý&[ßO?'À¥ëfµ?•nž€Ò?íÙO"c=x?¬Zèš7î?˜ÅçQô™Ž?¢»æò#.¿?¦4Aw°?¡öÍ úd?êi¹Ú¬´T?±q­Q©?¤—=P›ãq?šÔ*X&?Á3I@ï<?¯Ò3{þm?ëfQÊ¢?œ˜ÁÈÛÓ/?ªvÿŒxÚî?TˤҴx?ºM³*þö?•Ë¼2t7AGN4FGL J0807.1-0541?æö­qùÓ§@,VߋÀ9Š]ÜTÀ;³›ý÷è@v©÷	â,@ÌúÕS"?«ã!€‹ß$?¹"€z䢬@
 sÃF;N@
¶áQê?î¦xÚÝ0È¿ÖE—¤Kú)¿äp5݇…¿àaßyw»¿åþw4ÿì6ã¡¥¯AGNbll3FGL J0807.1-0541PKS 0804-05?ïæ³á¡ù˜?XÒ|«¡Ô?4Õ}OÎ 
?$F< ½'n?f±n–Æ^~?WàrÏ0üa?ïت"´–[?u•­CÆ?H'[SN?S
Á¸N8?p¥Ò=¡4'?r®¹0Á
?ï‹ø'ðª?¤b«´äÐ?iù±ÜÚT«?rØæä5¬-?†½•sÛt#?}æ¤#]?³?ï¦ ÍÍJC?`Ò>4›ÎŠ?]¢Ú—Z	??^óøU'?'Ãq2‹C?^líÝ;û?ïÓ¢<çx0?n^#Œ†º?8Ž	üL÷3?/o[¢Ÿ<=?t¦ýÐS¬?mÏô™úMs?ï•À™b½?ŒÓ¨à¾¯?^t9x?nUÝy7ºZ?†ÁRlʳ·?‰3$MDßâ?ï^mÚ+¸ž?ˆJ]Æa±?qu\aÎ{Ì?xûv´Œl?©ÛJðŠ?ƒøiÄÐæ?ï$Êș?	?|'Çù)ì?r­ß(´?[‰ž?–»eò"FÒ?zW«¬!wAGN4FGL J0807.2-7630?ïºKLHqÎÀ69†3‹HÀ:‰: >BÀ<pâkš'Î@ÁnØå@î€F}?ÃTAöš{—?µªZ±ý>?ò0œë]±Œ@	ÁŠŒ5'ï?°	/(·";?ï lf±¿â-颛uè¿áª}?Æ¿¿ãt¶‹Aè¿éiõ1oä"AGNbcuPMN J0807-7629?ïù"
F­?8o	Φ;?`EFzr–?ª@vrt?HÃH~2G?6ULÙ\ÖP?ïåíÕõ¯?lJôÔS'ø?5¯ï#hU?Aå 	ÃÃõ?g¿gsÖ?hì×( R¬?ïÇ:øµš?`Äâ6Ý2?Nü
ÌSòá?5Öð/"t?xƒ<¾÷Ë?_+S×Ñ?ï½q'¿_Ò?YR2PÙè?]›£Žë	??ùa؉ö%?yàuÃÊôF?WÝüZé
?ïôü	‹?C¯Ç–Ô`{?-´ayþ? yÀ‰ü¶æ?RQnrjv?AeÄ´Tp?ïÁ°(ý$X?TÜä¨‡?A¼Æ£NÕ?P ¾}[üÒ?|ðRÎÝí?€O/*I†…?ïª,NVi?kyw‹ø ?Vó&ˆÁäH?K^Ø×Dv?' «_D?h™mê‰4=?ïe÷-û?sÕT/>?oÃ`39ÇÜ?Xp%#ÊcR?Žž:Q'O?r'ã +4³AGN4FGL J0807.3-1954?éÃëUN@Ôó…À;e*ýÌÀ<r»H@
²@ØhOõ‹³@V—:*?Ë"-;øS¹?±åޖ£Åí?ëV—¼IÇÊ@Ò¡ÍðŽ?ïï"Ê/d¿ä6A¥¼½‹¿å²>àæ¿ä"8säÔ+¿ÔUÞXæK¿ã!ÂUO"AGNbcuNVSS J080722-195218?íJš
?®TÇæ/µª?^˜[H'?PÈ{)sÍ?¶Í˜§:ÈÒ?®³–b?è'Q®|k?ÀοöЁb?"uwï,u?‹È´ùxP?ÎaÅÂÂ]?ÀXY2vJ?íԚ1Ö"? cÂ|y¾¬?woCÒ	D?jN"È5õ?µÿ";G?ŸÁ²¸/¤?ï@p
݇8?oõæˆ
?aB5é?Er«Ï"?•É¸UéÃ?nðÎÉÓ?èЙ?¾$'Y_?o*/ÞOæ!?b¼bw"'H?Ï?Fð\ýe?½íÏü­B?à¼ñ–ä;?Ær/ÐÛ®?Š®à)€>ð?"
ÔއÏ?ݲYÅËs?Å["ª=Åw?èòÈùT(?«Ìjœ?…èóGU—?tpˆpÙz?Êä‹×D?«cÌÖí>?퍤¼Q?Ž¢Ê—SÉJ?v;轆òB?fHL£[_-?²4 ؍Ð?ß®â>AGN4FGL J0807.7-1206?ï!	±ÉU
@%ÂÂ7G"êÀ:~[ãU¥À<;yQ$µÂ@~!IÑ°6@K>WS£ì?ÃæÆÞvB|?ŽZYñ@¨?ÆѾ¿@	è,B©ï¿â®˜™¿YG¿ç²Á-Ý3¿ç[bA=·ñ¿é8'â3n¿åõæ×:¿ïÈc`øh\AGNbcuCRATES J080736.06-120745.9?ïõº]DºÖ?G¡Šo0"?"iá_?…¿nŠd?RJ˜ne';?F\v+Ñg?ï¿Í¨ó\a?‡ýªx)«?CQØîÆûR?S²ç‰½<?}®ðIÒҍ?…áxü!@p?ïj*fc"Ø?ƒÿà·Æ™?hc9'^"?qØëcš¿î?\¡ICôT?€Êº	Žç"?ïâu€?K Fÿáu?>‹4"c?"üAÿ†·Ú?j ŠÉ|Ë?II¬ˆVc?ïéD*?]1	…¸WÊ?+oØò¡?"5¸FcÐ?eØ]ð/?\s뷂
?ïXÐü‡P?¨}"ÞׁÖ?^bÖå?tCÕa*Æ2?šnÅ_º ?§Ý *b—3?îèJŒk2Ô?Æ~Zø?si–k·¤?uÉÂ,Ì?žHÝҒ?ž¥0Ì\­?ï¯Aú?k•ÿ¦'?TDW_r?Do­¯å÷Š?´¸Æ:ûi?h®OëÆÿ+AGN4FGL J0808.2-0751¿î¥WIë@*R¾H¥‹?À7‰²gƸ·À;Vd'PÐ@¸éö©?)@å*"8…?•e‰Ç"~¨?µR3S"|¤@ jvSCsó@¸[äWX¿Ä®YڑÜa¿ßÃt
6¿ãk–¼o‡w¿ãž4"䤿æï9©nù³¿íRuÚAGNfsrq3FGL J0808.2-0751PKS 0805-07?車ƒ}x|?‡/JOÂP–?T¥.éC›K?aQ"M~©?"J¹:Šq´?ƒ¹e÷€?ï§ôâÚD?<ÏÅù¿Œ?^‹œl6þÓ?|3Wf3^?'1S̾.®?†2‡B¨;á?ï™|Ü۞Þ?Š››Zªo?x'ÿG]«?'?žs™ê?z¯'–¦cA?~÷KŸêWS?ïéȂT|?PJñøåæ?;
cQ_½?/@·äwm¡?bԻ΋µt?KôE[ÿÓS?ï°+ó½–=?|Š¤‹FŽê?PlûU$?LדwQJ?ó@Ê<Ò?z¾r(RåÄ?ï+)¢ÌÚJ?£»;e<âã?lg¼DïÖ?|O‡§Q±¯?—
Ô½¿Å?¢Òî멳?ï|ÉOÐß?Žmœ?~쨫?…|€]‹á?'ƒIîX?'ÆÅEGÉt?ïËGÈÛ?p?k§‰ôÄ·?MØj0Èl?EXzÏr<?v¡gÕ±ã?hý¬Ù´\)AGN4FGL J0808.5+4950?ì}&/Oßø@@EA [ÀÀ:
é¿KÚÊÀ<n«ï³x@^'€L–‡@¨1­!5Û?¼µ#7èz?¾Ô»-½þS?ù‰žsóî@©A,p ?á?ž{«¿æ¶<½u–Û¿éfæÀ¿ïL´ÔQP¿ïüð¡=Qð?ïûûùáAGNfsrq3FGL J0807.9+4946OJ 508?ïÜZ¦ê?}|݌?`}"bwZ?{	6xú ?c(9‡ç"?cÞY3òN¨?ï-"‹H%¼?ÆJ'¦u?'ìÕ¸z «?he§Ì"³?Ù¹^`'?tîìÇ¿?ï`v(a";?…˜S¢]p?møŸ0Uáö?rJŒjÚÞ?2'
)%s?ƒ…Øì?ﳨ'Aå?gQ½¼«mà?wéNÅ®H?cðØ]5N?l"ÐbB:C?Qjûڀ?ï»z
÷Č?L4EˆÉˆ?x:à§þ<Ù?ŽY-)1¡?d3"ƒ
†?h')P"?í䫜Œ¤O?±dˆÓ»M?–4;y†\Y?£Q-ÑØ?¦›(~¾ß?¥Fw£CŸ9?îÃÉ`†¨{?"~GïÝçà?}¤¸Ñ)=:?ݎ•oí? Òàõê!?aøk€?î丟Ë?ëª¶bØ?—Á†"D¥?ô
|?ˆ¦]g—Õ?s;ìõt&gAGN4FGL J0809.3+4053¿êº˜6)@?""åÕ²OÀ:Zi¡"I¦À<yèÿ2z§@ög¢{•x@ü6ڇ s?Á¨wB¯Ã?ºzÈH-Á.?÷ oz@
6H°HÕ?ìø´¢¨ñ¿æ6¿áa¿èׄKS»i¿ásï@j(h¿ïÿð°×£À¿êëÒ¶ñ™5AGNfsrq3FGL J0809.5+4045S4 0805+41?ïïRÙ@Î|?T*r9³t?FDËoÆ£?B©ºmÙ«Z?V7èKCÐX?Mƒ-p†ûl?ïÑåÎ%'a?v¶Wéî•"?Ra'£Òt?aó4"mÿg?rŒ@þø?o7¤hËã?ﻣJ(î?s,Ä3È?]	­6Z3?aö+(?iÃ?zÎ0ã?Z?moD€=u'?ïÉc'»GÙ?T©J}°çŠ?dÙàÙ¹2?EXó;|	¥?páFB½?NÂ'ˆÞx?亂˜wZª?´¬Qúk
?'+/"YÕ?´¶Òù÷"?b·«¾–]?[DÊOèø1?»þYž?ŒÚ㆏¶?` Á‹c•?n8yÜvvG?Šçà'Š2r?ˆ†¸Ò€&?S큽?yÈÜd.Ò ?eç&uKºË?aršV?–?‡_¡jR
?vdÜ]Äma?ï\ÊÜi?wT«LÐ5^?€: Š°Ù?j·q4bk?ˆÁ,ÊR7õ?ošV\AGN4FGL J0809.5+5341?ÔQõf‰@@vQ ÄeÀ9OM½øôsÀ<w^o@ÿ½ð÷4@QâZӋ?®2ó'Þ?¼ç—~aYâ@¶î·`-@
+m—C¿á+}âƒî7¿Öļþ"°.¿ä­'Lž>¿â±4Ur"\¿è"âÀ*'¿ïÿûbâMhAGNfsrq3FGL J0809.5+534287GB 080551.6+535010?ïòŊ8R­?Ju/zU€?BB#ñ¥V?5½gpr6?QSä.Ä]Å?CtéñQº¨?ïàÆþ˜*?prr²iÃ?AWmû/V?J¦È\˜?jäöd½?m¼/㗠??'F?€€ïc+œ²?pÒÕbA?y¦‹'È!b?}àÄ«2¾?uµWV#[?ïö¿¶Œ?3td:9Gz?*²©¬ß=è?øpábö?NT}=ÆÅ?0ÖÖOsy ?ïêÜÓ¿?UXl‰³K?H_€/2"??¥´v†?^AÞoS?Q.Bv²ºÙ?ï¤-ÛÌ?"'Í׍?VÇÈ`igÇ?cEðsŸ»?">ýòÚ?'^‹,¹²?ï\»Ív?Šˆ‡Š…?{¶b?)íúÅߘ?‹mΰ>Ü?'§eEeK?ïéƒë÷#Q?Pڀ~'o•?@Ä:4·Ë<?0NCwèN?bKr¿¿æ?MÅD̵ُAGN4FGL J0809.6+3455¿ÛhC"Ü@>[=ÀTïFÀ:—öÀ¼RÀ<…¬bäÒ@ ìKœ%?ü­,SE!r?¹½0EÃ?xHÝ%Ï6?±o¤'½@çèF¥Ö¿?ï…[ôó]?Òà™ËW'¿ÝC­iZ6­¿Ô
ÿx›¿åOoù?·î÷€:ß
AGNbll3FGL J0809.6+3456B2 0806+35?ïàjëӚ"?ZbS8ä†~??ák²=¬|?+M4÷'%?k˜æ· ½ë?X{¡Xw1Ý?ï۸ߞÐ?pÁÇZþñf?FB{›
?Q"èÜÖ?olv§Mu¢?k Á˜õ…'?ï`>?z"ÿîæ'À?W]&‰E%?@™ú:ŒÏ?‰_áÎ?z<ùd–;Æ?ïq<ÓÅåR?iQqEí<?k§aÈ
à?JÃïÐ}F?ŒÍa4\ÚË?gñéYzæ•?ïÏadýcK?g'H9nÒ?H—Ï­>Ã?6ܳŽ?u<iüì¤×?flL[ž®?6¦Á\?…}AÀ?Sø!{±u?`8)#Ô2T?‡Ÿ.»>¢?ƒ|ýo†©?ï*W1ó ª?†O©Ñï"?b?
ÐÛÌ°?_˃Œ•Ú?˜m8¸£5?…sL0Å?î'6B $Ò?ƒ ípéD¥?\,éOŠ?fא%ίõ?£˜Ä֊ðò?'Bß?!AGN4FGL J0809.8+5218¿îó7æÝUl@@uÂôÀ7ßF€"À;WFG.@ѹ©™è?üúÜà@G?™úAú÷,? ¯·=C'a@Æy{ìài@/®'MoÊ¿ÈKÇ©¢PL¿Û ÿ-C¿ÝùVÆ'!¿Ø`Z³ª¼Ø¿à҈˜ÀUÆ¿ØÿŠÄê€<AGNBLL3FGL J0809.8+52181ES 0806+524?ïñ©Å®÷?iÂ'Ðîk?ØÿJB?¼ã/œw?Zþóm‹_?i¶"c·íe?ïÞYDZ8?lƒ™:ò1?Aû@ª[¬?IGrÕÑ
?m(,:ñn?hŒùÃ
ýã?ïÏ±Ù?…1ë{Þ?]‡‰+ÏE?i$5'+‰?…›"s.?€|*=?ïéõœÏ®ÿ?L†1€A¦{?"w'¨Úì?
GJÔXÉÛ?dâéäö'V?KÝ'ßy´?ïãçzÅer?g@³©,5?%ˆìt'Ñm?Ë.A,µ
?j¿öx‹bº?fÖû²ö?ï ^'¨*ù?"MBzáa?Q!4YÙ"?_ w<ÉF?…¶·rÙ¢"?'Õàç"?M9ˆ?†qRb)i&?X­Íyì#?]'Þӝ¾ó?Š{'»`]?…†ÜR¦Àô?ï֖3Lwl?d½b4›‰?05B—˜?$_­×Gc™?s«âëë7?dP!DAGN4FGL J0810.9-4926?妜bKÐÀ!8÷‡‹zÀ:·SŽÕÀ;ó¥è\uL@'ªk¤@K€œr'î?Ìw›Žy?¯ðRAâ?äSõ`æè?ყòͽc¿çµfI
5
¿ã݄ªõ°¿é…Áàà€¿Ý8Îø ¿åÇM1:Ç¿ïØ¢žP³AGNbcuPKS 0809-492?í:Š"B?°ÏT­˜?tµ$ ¯s²?s/À˜O,d?¶TSâÚ7?°l,Óä?ãÃä`è"?Çró\ÙtÑ?9oÌÝ?"U›§‹«¸?׀.¾ÚEÜ?Æôîc[ý?ëO¸˜žƒ?¥»=¼Ðµ¢?ŽY
4qþ?ƒ¼Â&¢Iu?ÀیÊ'¦?¤–A}&[?æF´°Ýi8?¦d—Uö6?¥)"®‡Ã?ˆ'éB?ÐÍfâ@–?¤äQ/¿Ø•?è…@èc½P?Ànäw–íö?"‡1oá$Î?'©›B×l?Ì¢‰F)õ?ÀBrm}(l?Õ£¢¿æ'ú?Éó1\æ­?™ªnÇìÌ?¡nÓ.|u?ä`Û)±Õ%?ÈݜLk,c?å'@yí¬Á?±ßæÙØ?ŸÞY[;?3¥…n'?Òߞ¶ŽòÍ?±Agû?ڃU'ú5]?²¥&°6÷µ?³…'̎? B
L¶ëN?àM²Ñà??²6œâ2ìeMIXED4FGL J0811.0-7529?çoÿ×¼À5r=_ÜßjÀ8~é°2bSÀ;ŽÅ=jÅ@ÎȦ!'L?üûõ)hÄ?£pî!'ºQ?³@ÒÙb@{Sþ"Õ½@	.¡Kϖ?ï`ø0'æ¿ÔžÜÏyOw¿Þ_
agy¿Ûé¯Çˆp¿áD…Àô§\¿àW}à€ˆÑAGNbll3FGL J0811.2-7529PMN J0810-7530?ﳎ&7»ó?~*L#€øã?Xºô'Š4?Xvæõ˜¢?€ç\Uû?{CƒÏ¹)m?ïhow×8?'Üêù~N?r0Ӝq¨ ?yþ"jnö?ŒËÐHۘ?‹ê×â›e?ï1"ßo´?'‡Òªƒâþ?tÔC¶Ó")?Àã#63?"šS¡`?ñÆË8ʍ?í2šÔN™?;:ì'?'ØiŠž".?njy(´vä?²èPÄþ1?‹æçŒ3 ?ï†b?–ëÂ{þ½?oI.$?o;ãbêË°?˜nA¹ú0_?"ĵ$…2"?íùh‡ä÷w?²ÌŦ¶å9?–kžWÆè?®J5'[?¥3¨Y="?£€PË´Ø?íÚí®2œ¤?¤™ŸJsñ³?"!&ñ§fÓ?ˆ\°#+¥·?­HÛ`ðM?¢® ü?ê(kħÃ?¢S§\zÕ3? óÙ;|9?'Î×9e˜?Ã" ×_g?¢«¸áüAGN4FGL J0811.4+0146?æL
ô6ƒ@2ìAÝ"À8ð&n(ÓÀ;nÇtž8@G4 ñ|¯@üÉð?˜ÿjÙ½¡?±ž
áXä·@]û¹I@³¥ÂqÕ¿ºž'úb¿ÝxÞ8/¿á¦.ÓR"¿à· ÈÍcÌ¿æHùµ¼æ¿âD`ý›Ì¥AGNbll3FGL J0811.3+0146OJ 014?ïì@ÝÀn?RY[QƂ?@»íQ€â?3Â×J´[?_rgÙ´û?NcmTcÊ?ïÒåÀ5–?ro E"r?Mï¤Iƒ—–?Xñ¤*ÀÀž?rÏ+b3šÅ?o^`(46?ï½Y3ÅKÆ?zµ¢Z~?dì?›ÛÅ?sÖ8S<?vÝF:Β]?qÐ2rñ÷˜?ïæÒ¼L#?M¬–Q''ú?8ˆfxÐ%?"
yï­U\?fA[{m?K7AÁè^S?ïà
ÜýÇl?_¸Y~fÝ?:œ>"§OÚ?-à
®8ì?l¡›ú·?^¤ Ä=T?ïØ*+«?'‰çz?^¶Æt—?rKe7
õ?ˆhwø/G?»
£$ß?ï·y Q?€Î§ƒj?Ó?d…"u¶š?tWŕG9?zužÙm?{àÝ>vÀ¡?ïËÇßÛ¥á?dwíÈÕý9?I.µ›ai?:¶!vRÓì?vö9N" ?c!t 蝮AGN4FGL J0811.9+7847¿ï顦¥¾
@>t‰ãC0×À;Z¨®àR¼À<£¿Ü#å@úËܑ¼?÷Ud;ü?á"r&Ž	?æJ 'l"@Ž{Xeó@gî¸/ý?ídIáJˆ9¿ëÇ€\±²¿Áã˜ËéM¿æ¤á@¢1™¿ïü#åGî¿Óè5=ÏnhAGNbcuNVSS J081307+784308?ïZåBÆU?'"c$Þç?v'M@¦?rhÞì*$]?Ž7æÆÿös?Œ¸÷8ùIA?îè¨6%½?›kù
͑ü?"ú&Zl÷?‹e‰¡ÈÊÜ?˜mæþu?'3'´éz?íßeÏ£Òê?œÁðEæ™?˜kO—2…:?'ja…œ…´?¥Óû5ÞÎ?•åÏü¦?íe!Ë_m?–׫ÝoÛ{?'ó-	$£B?sÑø|qI?µ^qQžO®?–XZþáï_?î;ÂY4m?¤tªsqìË?'wÔ:
ô´?'lÃúJœL?£ðM%9Û?ždùÈúÇ?í2Àå
€?·]"ä'€`?˜k:™U'^?§7VaHæ?°O*0ÔSí?±ÅcIký×?ì`̯¬½?¥|@ÁŸ?¡ù7éDõ?•®ôoŠ?¶]¤®"? 1'Ùä^?é·Úe¢ØC?°œÈ¼Q<?€1'Ѿk¼?€¢þ¥i?ȃëÔÇ:?°Ž""©pAGN4FGL J0812.0+0237?ïçk²ç¯@3ÚãæÄÆÀ9ðËЮÚÀ</°r#3@ Îý~›f?þÝΗ¨'Ò?¶Éš'ª·¿™UpŸÐ?s?㝺|h0?õ ôg˿1f™'?î
üwµCC¿âÆAp㘿Ù*»*
Ä¿àcJB~Q¿Éy—›'˜AGNbll3FGL J0812.0+0237PMN J0811+0237?ï·r÷³6?|jïЊ?VDü(	?T°Á±öf?~µEŸ®°?x°¯9XÜ#?ïcÆΌô?°®PfÉ?vAèK¼¬?~³­ÅX?‹í‡¡WO³?†9ñŠ¾¬Æ?îáZvÕ/®?LçMýE?'N%=@?'†‡2Md?š­¤ §?ˆÊò­2õ?íYú~Ù?ŠýéH…4E?kͧ"ä;?}ãY8¥íÌ?«¸Y´G0?ƒâ†wôÈZ?ïö ¹Q#?Žì´É½ý?fã¨Ãòu`?`»é–'F?ŠIm•n?Ë 4©ð?î
Ãä'?¬Õԏ75¹?'ó»Ð/?¡RÄr0*2?¥EvCã‹~?¢Z¤ôÉJ?î.ZwV	?˜&~RÅ?‰ÌQõ©S?†ÿΖvZ—?¦§D€^8?"™`<?q?êCù¦Áí˜?¢,œû؁?¯:'QIê?• ‡%vý¥?¾C2€lK?œ˜ïè•1(AGN4FGL J0812.3+1143¿æ^¶!m@©@76OD
ñÌÀ;«°óRsÀ<‹Q$µÁî@ͳLóùŒ@ÞÖ4T›c?ÎAƞàUk?ëqÈÅ+C?ñlÐÈÚÏÅ@±´›Ó†?Öñe]|ÝÌ¿ÔÿcÍÚ¿¿çût_ÎFÊ¿ä#@v蕿ïÿÉ
ûkF¿ïÿ–þߙƒAGNbllGB6 J0812+1141?îª^Û$ç?Àgb/'c? tRLÓî)?¿:â-uó¼?ƒ—Çv?˜Æ!¡‹6?ï†Suë6?">$&
?k²Ö²ûԛ?pBþÛÿKû?‡~lèAºŽ?|í/ðŒ›?ï4gU4÷?†­½°'º)?xà2´€3?wòþ:ß;?"DFŽ¬A?€©ßv@x¿?ïC›ªã:o?m1\Í@$/?}Ï]…µ?ZÛimǤ?Ê	¤»?fÞ»!'¼¸?ïG™[$L?Œ)K]3}T?ƒ_ežú?'òåƒOõ?Šº¤äÍàÎ?åA ¤ÉÐ?êDµ?¢K:2xD­?ƒJƈG/<?rÜ69\t?¡4ì²–V?š2A4—{ ?î|ËÜіz?'1Û?ƒÖPÇ?|ƒkäí•?£s¬ª¦.?é5䎣?íãÕª–ìì?ŠyQ›@GJ?"r¸«ÃíÊ?{¸'£?¨	IBïX?…(üÄ:AGN4FGL J0812.5+0711¿à
½S©d@5LP&‰ÅÀ:Ë7š¡–À<qe/.Á´@wP3:@
¸A$?½µ˜'ԅ¿‹R"Sba?ÅÀ›{œª@ˆQë…¸?ÛÏa×`z¿ë¢ÎLT¿æD‹ë[-M¿àâ4½÷ÇÍ¿åŽ)Þöšü¿ïÿ¾úAGNbcuMG1 J081238+0712?ïéŽvBŽ?cíÃÊ 1?B%·nƒ2b?;pÉ}JK?aèr™Ðv?a«`¤4?ïÖ´§3'†?r IËíÐ?Ej>§?S8cn
?qóúÕF"?n>føô|K?ï¦Hé†?udìlèõ?T%ý[†·?C)‰áçR?ƒô9H,0ä?u-t{?ïڋñݟÐ?PúêˆDÀ£?Eùù]̝?+ãL¼êè¹?oõÏ™mh?Oy÷$²lL?ïÏç)ÖyZ?pêç~ü¢º?Pœy…ø9?DZÔRïè?tþl
?nØlÄø³?ï—$¯a×á?†=êFm=?UA6{œ?b¶êo'9?‡Ž­R?/C?ƒê{:¥?ïOö-Ƹ?ƒ(f£e†Ö?cSÓZ¾9"?gÁ-%_Ýw?"–Ĩ)ï?'Dì§?ï‹ôH|Ü?pkß:MYÖ?aÿʔ#(?P`
b0_?ˆ'ûcaM?nþ+•ã2AGN4FGL J0812.6+2821?æ,IqZ'¥@=9Ñ쒛À:ö ‹Â[À<¨7Üæ @ƒ	ðï–Ñ@&÷ãÑÌ?¾r`ßW®¿¨õF'_/)?îA|7@èÈ€ÿ?ïåÔ`Û?ï½ö¥ä*·¿é˜+ˆ¿ãz?–îÄn¿ÊÓ_ãëL¿ÔÏÞЏ²AGNbcuRX J0812.5+2820?ïƗöΠY?zæ³ß?Oв覙F?K[˜<F?x¹îö¶‹?x¡¦¬õ:ƒ?ïä+÷æ½?i¿•ø¶É?:ï"Ą̂‡?Döäñæä?hv'§Ô»?eѳOnñY?ï\P"SDÝ?‹X!ÓZ?dK¡ð$r«?q­×)J8Í?'ìy=î?‰OøiGg)?ïÛÖÚº¶?SdÌ	7Ê?MÄxz1…1?;ø1ƒžn4?l¸g®2)?Q¨eb¥ÿ"?ï…Öö¯¨?Š…Û£^§F?dŒþ|"wT?gõ±DË~÷?‰kÚ¥š²2?†xؑ£—O?ï°['îvã?'juÏmñŠ?JŽ"ž^Ì?YØúƒònï?'@2MAÀ¬?€ü="}ÿ?îóúF5L?"Ÿªè'ó?hølC8N§?sÎ)TsZý?ža©³ÛÏ?'è[k#é?ï‹vô(0v?tm{I‰?g"‰©%l?^´fŠ\¿?‡= #h?rŸl÷5AGN4FGL J0812.8+6507?ïŽÍžaˆ@@y§~^ª°À:žÌZ·»À<š€ÑK·Ž@ 'Íút@wßÖjÛ?¿kÂ_¥Eä?ŽŸj~y?ÐîOá?@>!œÀ–?î)Ý´{/¿èÜÏ^w"œ¿à'ä¾Ûó[¿ä"¥¡º¥X¿áԦ˱D¿Ë7Qzñã³AGNbll3FGL J0813.3+6509GB6 J0812+6508?ïßL[΀?YŠ¬n˜ñ÷?MŽÙ@½+?;ó"ÞYñ?iOî"e´Ð?V/­D)Ñ?ï›Z¡-¯?''½¤ën?^²¿
S­?böjm³ð?…SÇY½®?~-l(;˜?ïw¢²X=•?v§UÐß.Ž?a"iššð?H¹†O°:?¶8ù«.?u"6d©?"?ï@ÏáTCN?t«Q^`ÃB?x»iK·Ó?Wš4j?'·~"D@?t
€‰æ½Ì?﩯ç#?vCû ùÌ?bÞt-97?SÛøõÛÊþ?€Ü¢­guf?t<ø'¯?ïßÂ{n?—&Ê	È–?kqRm€?r]ͨ1'?œ.»4kd?"ÃTdA"@?îå‰ÙKúï?‰Ë'þÕ?m¹€Ì˜H?cÑ«Cé "?Ÿ—"µõ ?ˆ3=«}?í©>]ˆÇ?'hQÍ?'ï)ù5¦ú?zó1‹¡\ÿ?¬xh‡?':[gýÑAGN4FGL J0812.9+5555?Å7‰àg@@»3ÞLQÀ:þ'œ&;ÔÀ<¼MÑD*Ò@ ž
Lµ@CHÚde?ÃMИ^[*?"V±^ÿŒ4?Ђp½Ø=C@Àõܼ?ê80Èõ§·¿ç_&DÉ¿æ€(^ÃÚ¶¿×ì"é0°¢¿âBÞ¡áf¸¿ïÿ¦¶tFAGNbll3FGL J0812.9+5555NVSS J081251+555422?ïƼŠèÚR?Œ6ÀzfÊü?T‹­BüÓr?dCI9Z˜Á?w~Ï3ôj?‡ÆXdM?ïÛZóÛHT?nÚ-?rî?AI­Ôð'J?HÁß@ ùÔ?p)PJ4~?kk"wÞ?ï'AáL?ƒÜuþ´!l?U	ÿEåyV?TE7ï´?‰\¥w'A?ƒ›h#Éi†?ïě™Ë
?Z~žQÅ?Wô'
ôm­?6Až?wµJ{™?YÌè‹M0I?ï¸dÜO?|} ç,$?WOõ9OÔ?T¶Ò.Ÿq?}ù"Ô×hø?xFMfH?µDoñ?ƒ[XJTÇ?Pïðï½üÉ?Yl÷ˎ>^?‡}ԟ²•ò?ÁOt`?ïL™ßm@ÿ?†±³¦<¡?`ޅd4Q?a"mwNV?"Pólܒ·?…Š÷L?ïE˜yø®A?v•±&ƒða?sñ@¦	©?XdL"Ýäù?'†ôq«y?v\@¡É|€AGN4FGL J0813.7-0356?ïò¬?Ž‹I@0Jò"z–À:Ê/•ïÀîÀ<p¼Åd@!T(Ì'?ú{¬\ë?Èôî~ù/V?Ç`1Ùkì@J¡äÁ¶@;DI[Ë?ÔC¹"4$Ë¿ålüþóg¿µ…(ÞÆtn?·)£dm­¿ßüEá5ºw¿ç$8YáAGNbcu3FGL J0813.5-0356NVSS J081338-035716?ïűŽi ?q«Ÿ›X§?Qˆ.…¢|?FFgf.·*?xÅ-HDÎ?pÍ¡:ý?ïi½',-Ÿ?Pà&͝x?eK%Š?gÏd,Öqï?öqS,â?	Ôۈ(7?ïL]8×q?'"Ðgnº?gjXe&2?\Êëý8Ø=?"'+¶è	?'P+7!?î)¬Æ¿cû?…;+'ÃFð?z°"`<ר?^Ð¥D«ª5?ª/D|‹á?"k8ٍ=?ïœ|°TÇ?±"WØ?_—x?Sþ&ywùS?…S$#Җ?|Òä¤ÿ?îewû(½?¨­xëñwž?z¡¬34jØ?'OŽÛ¿÷¯?¦TJÈ	ËY?§àÈõUA?î†[lƒr?'Æ͋6õø?s͟øÕª?l€Þ"Ö¤?¥ š7ûÏ,?'²ã"Ão?ëËÎäÃÓ? YK2³z?aé ŒßÄ?~H£TÿÆÕ?À*²2d"·?ŸÎí¤¸ÐyAGN4FGL J0814.2-1013?êË~Y"é@*m¾]ž@ÈÀ979_JÀ;ødÏ@ûÃ	€@•{âÏm'?¯©¨|Ø»?©^v¿
R¥?ú±ÅÅqŽ¹@	½Õ{G"?ïÿÿÊPË¿Ú$'óÕz¿áÒ¢dCvw¿á$Øâ"Äö¿äŽî_ċ¶¿å›«–òAGNbll3FGL J0814.1-1012NVSS J081411-101208?ïéc²ñž,?en´¨8¤Ô?+´ú+ˆ)o?"M|n3‡3?dàýŸE¯?d¹ÇæÎ˔?ï«À–Ĺ>?…`YÍtê?\C»õnÁ|?fÇ`•ÏÐ?‡bÃTU?'¥ÛX@2?ï2ü…æÎ?Ž¼V¥+²±?cÜ3·¸?fhM×YYÂ?—>½ËGÕ?þÙÁ%Du?ï8pýX?q("sgõ=?~V×Ób?[š{/?'XʯV¾T?j''¤		–?フ–ô?zîV"—Bn?Bbk!Rû´?9"€+üVÏ?~mgo¤ud?z,â·Ý!?ïŠñÚ×? Ü6pV3¦?oVjFýå?‰ý	úp?š£Ô'T?ž´ÌìPwq?îêÇ	Ðtˆ?"$θיÒ?kh$1Ý¥'?l?íK
à?Ÿ::æFK?"SóĞ°#?î&ÒÛb?ˆ‡l…g^?'Tí´²?tà5&«Ïø?¤s¹TÞ?ƒm)@n™·AGN4FGL J0814.4+6926?ÌBUèd@@C3‡	WÀ<0€sWæqÀ=+ˆlJ«ö@"òÌ!V;÷?ú	‡¶Õë?Öxë8Ȟj?É¡ú{±§,?öD?Àà0?ÿƒµl3¿ïýv¸ÄL¿íEIJ̬ì?ïþä­³,?Ë¢Ú`S¿ââÝ°IßG¿ÄC/ÀAGNbcu1RXS J081407.6+692549?ï·uï_7¸?hH¹ŽHÜ?K4ÜÛf>?E"öÃNÀ?€qPÐS?òÄé3¢?ïŠbPúeÚ?Šwtä+?e·HMA?o#''è?ˆ#}èË÷^?…oȃʡæ?îÞì]r@?'RÚçÜ?yùÀêL?€¥âÙ¥·ƒ?Û°—ot?T2ñ¿¬p?ï$€\ªY?"LBåu?_1cK",?O2úQÕ?™|ÞF¥ë?q+cÎ?ïvåÕ\ha?‹!á?TàQ?N‡ÁG6	!?ª‡Jö&?Š{18Wƒ?îõ×wmP?›ÄËK˜YÔ?s®:Bu‹<?" @²	Ãq?œY''o¿'?–Æœ/kÀ}?î"
7L®–?˜"Èåü8?|–
Ñ`Õ?…M±"r'?ªLšì¸¢	?–ë''óÔ?í?µá聣?¢ªZ§?qIE¥ò߃?pTj;ŽE°?´í¼"B3?¡ç0Ý4ÒYAGN4FGL J0814.4+2941¿á?"hk›@=üGõbÀ:õl‰–WÀ<'@Þí`Á@ ³»Öƒó?þí@ÅÂíP?ÈcF¡Oš?²b["Ñ2ã?êÛª ¨»?÷*&ˆó?ïþР@ý¡¿éËßR,¿Ú¾/Gì(¿Üè'¯qr¿à姏%¢¿Ø¦á€¸øAGNbll3FGL J0814.5+2943RX J0814.4+2941?ï(''®y?šj¦<XR?F\÷Éé!?F0þÍá?šL¨,âê¤?š-ׂQ?À$"?™¯vø]˜?€œ'Í&Ix?"®Ø'þñ?–@·…[׿?"K³'rß?î|©‰PÌ ?›F/‡Ôó?lš,§Øëw?mÊ`
ªœ'?¦kÄ¡¿‰Á?š·Ô³š"‹?ì¸Á´Y¨?'~4?K5?'Ž¯v&í?pÖÑt-¤«?µÜ0GÛ?ìáa¦°{?î_pƒÔ>?¨¨Æ¯½¢?Q6BÙ?JAË©'8?©€3AûìÙ?¨Œ»oPh?íN:HƒÚô?°ï²­&?'ù\'I¦?šBÎS!±?°ÏÖ²ø¼õ?¬oÌBm¡?혍—©Ã?¢¨ß*‡?viÙтÀ?u§O2?à?±Ôõªmz¢?¢\<@•?æ"mYìý¼?§òž¢æ÷?¤4²Ê'¸?š¢ù¬¹8?ÐP	GÒR?©P=zÌßHAGN4FGL J0814.5-2642?áÖÙoêÀö@ªžåXµÀ:Ç!—)|ÑÀ<=ŠV/·~@tÿKû<@a$z2Ì?Ï«b"Y–t?Ó½Éd7
@ SŸºE@\—rÍÒÜ?ïœø^Kò?ÕÖ\îm†¿Ü±,]Vl¿æ«Ý¾â~e¿æ'ÃÉf¿ïÿÚ`‰,ºAGNbcuAT20G J081427-264422?ëIԖ+X?²U.%o?ƒ¹Ì‹§!?vد͙@¥?ÁßÊn?±mz¿<U?éI$¤O*5?½·ìH›­Ï?‡í¹Hº?‰ö…£…)?ÉiûÿÛ£?»ÚyÚGÅÎ?íP"FÑ? >$iÌ	?'[÷QώE?ˆy%œ ü]?²î›h?œN	ù( ?î-\M͂?™(þ"?‰sþ拠ï?fèÕ½Éf?¦Í;h©B?{`ðM?æì
4ÞN?½s9¦k¿?'ŸiðFÚ?…Aý~Ú÷>?Ñ
õö»Ö?¼¯ù·"þ?âWÙ ×?É3Äñ"µã?˜T½Ö쉡? >	"ç"ð?Ù̆oµz?ǽ¿¢±Š?êÍ¿7Ó?©Sn#ýÌ? 	#ÑQ§ú?'B³•–o?悠®¶·?¦(ž†r³A?ëqÚÃtM?™èp»U¶S?šD(n¡,è?'~»û£å?½æ—
ÎÜ?—z«MéEhAGN4FGL J0814.6+6430?äiÆPÿw@@šb=ú	À8©ƒEW"À<µê28a@>Èáè@Á£n.±Ä?žíC\B˜x? XÑÓFäk?þvk+Èç@/¢ÈÂQ¿ßLVð§h¿ÜgÇúÕô"¿äuð²…"ê¿ãsÉü7ô¿ä¡^E°Ž¿æ%ÜÓ«
_AGNbll3FGL J0814.7+6428GB6 J0814+6431?ïÞ5™®¬?¦y{¶ÂÖ?fÈm_†z¼?¦¿öøä?Vñ‹¤â™?S·™¬0l?ïÇðRª?uïÔ¼³?P<G•'?VA¹Œ0K?wøÄ÷ê%"?rª†mÄ0ø?ï¤^>Ø5"?'õÅMTW'?Xõ9"K?gGç¹üÕB?ƒÉΉF*~?'H…Ÿx–?ïê©)?IÈ¡žšm?RÙåaºè?;OÃ{•¶;?Y$ÈsŽ"†?@P‰`ǚ?ïç髪¾/?`5m©µs?AXGâ¾5æ?QE¡.ú%?cÀBuOs??X@L¢K>?ïk8Y|?žPƒ=F8?_"â©; à?miž•‡N?ªjÂٓa?Ž3+BÒL8?ï^CØ5Ð?‹.ï$²ß?]@<F»?ZT*ß­¥?'lã|=r?ŠtÏDR=°?ïÊð»áºg?fºy¼?gËs½±6?WÉðqël?mx×â¿z?]²PòGAGN4FGL J0815.6+3641¿ȩ̂çÚE@?ì"F{åTÀ;ÿ!³®ïÀ<˜­4
@-£ôfnÊ@[¡/?Ê_d©ø·a?·oÇäÌÃ?ï2 Ñœ?f?îÅ.S-,<¿áBÓNÇ
p¿Ë@%	#ë¿ê¸¬"Wé¿ÜÕ¬˜¥¿æv¯Æ+É¿ïþϞŽKAGNfsrqOJ 320?ïYaÈQ?Ž"16¶?f ™+J\¡?izh¡ºß?'ÿÊ~}"F?Œ>™5.?‰PÄ? Qu'ŠN?Ž(LW½?•É-"Pv‹?šx·$XŸµ?'¤ârÝ_p?m%ûÆ?•*¸a"?Š…ô÷
h?Š‰áÌ«m@?(÷äá=3?Žt·…zÄ?ìÃÚ¾'?' Ô[W,?¡½<QŽß?ƒ+ç	€?±'¡²Õ›?‰ÿºeæ?îÍüNçæü?™¾è¼3*?xÈà)Yd?yÞNªµH? ãéN?—3'N‡Ò'?ì€/«œÙô?´òJ±Â?£_
—&°k?¨¸ŸQìG?²NýWóË®?©'±ÓgÀ?í­¬õR8B? CºáZ%û?—u$ºây
?"ËåV¸G?©jžIû£Y?—e4OLuM?ç…K!2à?§Ti¶=ni?µùŸªßúí?œlìØÔï?Æî§
?£µ°"•¥mAGN4FGL J0815.9+2951¿ã½S4Qãš@>VΚ,fÀ:ûàÊ°'ÚÀ<q±6nQ@E´%¶óÈ@zvSCsó?Úz}ib?×r2aüõ4?ÿ‹µÆ 
b@Ùèú)ý*?ïÿ~‹¡3¿àLÞÕãÍ¿ÔôŸd3Ü&¿è¤N"áÉ´¿ïþ8µS3"¿ïûÀj¾º»AGNbcu2MASX J08153642+2950218?î0¨ö1†?£Wq7?~hˆFäT¤?x[P_Ë6?©(mUš›Š?¢éÀÜ%Eº?îÉîð|ï?—˜–#_Æ?Š'ck?ˆUÍÊ 8?™·Žb‰'?ŽCÆɓ€?î
Y9ê?™¹í L©?–΃ôh?$_..?£Ã,ÓK-?'2Iƒu£˜?ìŽoÊ=Pn?'Tmݬ'¥?š–ágëJ?ÖÛ¯c?´æÉUd"'?Ž…4AW ?íÉ:¤Ÿ:?¨ÑÞߒÛ?ˆgò1Õú?'u¤ë.ÿ?´¬·ãÄ{"?¦®ï÷\3?ìÓãÃo'?².XãÑ3?Ÿ,éÚÒ?¡Çyn}^?±Ÿ–«÷?ªeşºx•?ì2†üø¨b?£—{´»ºÕ?¢Þqc:O?"îà5í`?´üeÁ®i?ÈNÕ3?è"ù{ùÂñ?¨pܼ"v?£Ô#i?—Y8ÊY§}?Ê®¶›Kå ?§
ŽâE)âAGN4FGL J0816.1+4909?íñ[ï·U@@Ü!BoçÀ:·HIÑÛÀ<«¿2°Vu@=>ô‡|@-Ðãe–?À×h‡'üô?°åä Óö?ðbE¥%¾Ö@ùì¿0þ?ïÔ\
G`¿×ËïW;P8¿ãGø½Ÿ¤¿Þƒ.ž#¿ÞNy	×W¿é#7r]®AGNbllNVSS J081609+491005?ï×̱/H©?d}ÀÓJçn?S^;ÍÌ?Bd´rÄÏ1?n"0Äø{Õ?a¼±TSòÏ?︬§ŠÀ?tôC}êü¸?V,Ç[6C?WsT—ö
?~j÷Ïí¯?q¦ÿ#²Dà?ÒòDš?v½"šaJµ?c=Vü©ÇÚ?]wD·—iê?Š‡µ›e?s×ƎæÖ?ïEŠÇ!oÅ?m«•ÐÐR>?~.‰$1Z¼?Yàjëw?†	§›%e?i–5"?ïÀÇ£m,ÿ?io›: ìÃ?bG¹ä?Q¥·1´?vxQÏÆF_?d!'¾µe.?ï:&˜Qà?'ñïµÊ?h»l;"º?rA®x/Zñ?•£¿].¡'?/×	ñÙ<?ï*'Ipë?'+µÉўÜ?lçW L|‹?aD˜ž?—Ò[
4?€YP/ð—?íëìn—|"?‡ú¼SÓ?"Z§ì?zFØQW?§å'ÉÿY?…ÍL|ïåAGN4FGL J0816.3+5739¿íÔÏH/Í+@@ó¬Äï‰À9'—¾WÀ<1áÜ(Šc@Tåÿù @CrSÍÝ?¥ LâÂé…?¬Ò½–gÐ@¶ÖU⊤@¸õh¢UÖ¿ã~É3»o¿ØG"ÂLÁ¿â±ðrÄB»¿Ý"²œõē¿å¡…¡?*b¿à<	›Š4¢AGNbll3FGL J0816.7+5739SBS 0812+578?ïóÅ$$Å?Iq[#,0˜?1ž»£ú?"z¸Nyü?T–ÁG?Fë™ñm`?ï¤~FyX~?éñ"<?a«14Àýè?gÒ7±+¸?'u¢úA?|à‹
—D¹?ï¾âÇh'n?sqÎI?SHýA®$?Z'][?Ì?{¼\ßÎ`?q¨JåàO?ï—¼:$?eÛ­N¦?to úq'È?U"f'y¶?€@j)¿?^^¥rÚÙÑ?ïæ×ÖHÕ?\¡•´Û?Cïºî÷?6Ò]ç÷lï?df%e¥)?Xesq»ª?ï GZ~óó?˜Õ'[˜	Õ?o÷$ö?É?x–ã»·ŠË?˜5ʦҞ?•ø'ëƒý?ï•DД'ƒ?{xÖ#bX®?\]
?cAIö?‡#)ì0Áô?ywE¬;™?îñw Փ?‡p
jlNk?Š
ì]T?ttWn?"ÊuÛI?€míÈÄæAGN4FGL J0816.4-1311¿åÂ¥ëÑ8±@(> ÿT–À8ŸªúêíÀ;Ÿž¾œˆa@èð!Å?ü®»iÍùó?¥xÜI'Í?©Ñyž–Gn@u¦uJ/@ÆÑÜV,²?ï÷$ŸF¬¸¿Ýƒž›3»¿àŽ¡¹"ËÝ¿Ó禆轿àce•†¢¿Ùf=̔CAGNbll3FGL J0816.4-1311PMN J0816-1311?ïá"˳ƒ?dˆCŽÕ°H?-M‡)û?!ô‡gàvØ?m	ž®y?d'fš¡Ö?ïÏÐ÷&Ë?|}Œ gä?I^ФoêB?S[±¼±Ü?tëªv¡H?zg¹ ÂH2?ï_üôüI?ˆ*ivk`.?fvu»Œ%?pì–†m?'1®&X)C?…¼Fè}ʊ?ïs~@¼w"?l]¼L©w?\X¡+/?ö?>oΡڜ?•[¨d'?jý™ŒBô?ïÍD.-9õ?r*³¾?9W/éŠ?2$iu%"?wÈwU\Šé?qØ"Çô?ïe_ì,l"?–'l+wR?_ÑN½®pô?p‡u•Yt?'VíŠx®?•`½ÀÈæ?îàïOiÛÍ?•¿‰d´¡?q%R
(³"?x€Bâm?Ÿ˜ÁŒº©ƒ?"‰…"?î¦^¯@}|?‰H-# W?q0ÿÚqÍ?[§.Dsu?£vîì(Õ?‡ªhS8|ÂAGN4FGL J0816.4-0007¿ïôP7-œN@2Å3	AÈ!À;+÷­K'FÀ<y³J@å´Ð+Ò?ãÚPx¾W¿?ß4þúÇ[õ?ïqèEÏ?úΘ´—Ká@帧ü³Å?ïþÂ^§U¿îPªJè¿Áb]åc¿ËÑexTÐg¿ïÿJ=eç¿ïÿÿ>¹úAGNbcuNVSS J081626-000559?ëmÁ×{Q…?ÀV
ðì3<?YåP[Ÿÿ?'ïx뛑c?ÀsZNÄÍê?¾öÂÿïcû?î ª 
ȗ?¸«¯Èd?"â·têÆ?©Ô…Ir¾"?£íl¥PÏ)?±/¿^›?ìn3¿£'?¥å@…ì?žoÕ§œ#¨?•fV;Äþ×?´òlœ‡öß?¢"X$:d-?ë®F,'¹?²Ró…	?}å.D?vqÌçÊã?Â̾äÅ?²^™†æÒ?él—î–?Åç·\z?•ŠSõXXÈ?>±;'Õ5?ǞW!,©	?Ŏ
 ?ìD‡âj¡g?Â-ááB5ì?œùq/̕?«á_¥Þʜ?¶d¥'3¤?¾¦ŠÈ	]f?꟝=#]8?ªk
ghÊ?¡ ڑ›Ø?–ðÜþF?Á9Teïj?§…çRb?é˜aqpA?À .|G×¹?tÊAÙq|k?€3°ÇÍ?ËGLky±Ù?À<ÉⷛAGN4FGL J0816.7-2420?è(Ó± ÿó@'ܱF^‰À9މÁµA–À;ÒWF7ò¶@1f]×÷x@Š(ãN'?»a'þ0-V?Æjsç-v0@	¯å†6a@ۉ–AJx?Š‹h(ˆ_`¿áU±wÜ°p¿ç8Ò¿€#¿äi+<Ĭm¿ì~Ø;•Ø¿áâiʀAAGNbcu3FGL J0816.7-2421PMN J0816-2421?ï?öÅ;*p?ÏïJA?ìžK6Ù?|ÙqÓYgP?Žˆæ3ŸA?‰¹è>ç?îÍ\Nàb×?¡+[6R9˜?[xy!u¹Ê?hŸ‹îW®_?¢NwJMüÄ? ¨jik®™?îå&M¼Ÿ?^¹Æè‹?'ŠûSðXr?0‰}o?š¸¶ÛÂá?‰@¥¦\?ïZdku«?lé	¸9ê?mYåM›ð?On¥þÇ?'5å‡\??iÿ
ؐ@P?îX®³ÃM?¡ŽÐf*'?—`Ò?Ìu?"=q|Nm?œÔXÿ—ó?•µ§š¢Óá?í
䏷?¶q×¼G¢	?q'¯Q;?ƒÛÊ©wC?¶~u職?¶'D,D?íÁ&sX?žÚ™‰ÁnÒ?•þ_^7ØY?"#¢cÆ
?¨îoÖCò]?˜cÖÀËʊ?íä¹rIjú?~ÄÑ⨅?Š†2+Ó(?rj,&J×?«ÜN¦"?ŠQl`#ÌÑAGN4FGL J0816.9+2050?ËSÌ}>@;»ä›«—À:•"¿e=À<f:N°g;@·ëm÷ªF?û<¹t*tH?Â2¡èȀã?È×(ñ:ë@Öoþ•œµ@ãbý%Z-¿â'úÒD?ïû(Êúd¶?'½¨d-ٿӆ÷ µí¿ãð6(°ù2¿ãÂýuâlAGNbll3FGL J0816.5+2049SDSS J081649.78+205106.4?ïÃ¥ê	ôv?t¨#òŽØi?h§èÿ—?c·kd¢?qÙr·E?kÖw.)oû?蠟lô}ž?ƒ€pe´3?fqÓÞ`1g?o§ËóH`'?9¯Æy?z´
×ϳ?ïLêŒPZá?‡fC½?yͱ´M'?~£þ¿9Ê?Þ"Ó7?}­\ÆÖ±?î­§îq?ƒòš:ÇF?<Œz´÷?nCþ»gË?§F`àóÿ?€œAM(?ï™
h
Û`?{i¼C×?yÃôO?qd¯¡R©?y·ºB¯"?obÖ3ßÉ?î÷®«W9Ö?œTÇØqF?bS	Ñá?‰·'™Q?™*Qû.æÇ?"Š£yŨf?îÁþ{à:?'p'xã͍?…é´¬H¥?…kàè¾&?œêÅÜÃk?ˆ²SÚ´>?ìÊæÀ?œù;O=S=?šüQcŽ´}?"¡J€bw?¸B›Â9?šœå³¶kÛAGN4FGL J0817.1+1955¿æojŬÙ@;rÍáŸÂ©À;JžWn{ßÀ<£ô¬å¦¸@!±=®6^·?û'êÊä•@?ÏtOȸ–?·ùÓ;PŽ?ꖎý‰X.@Z_Çæ´¿ïù·FRʨ?ïÿü9¡â=¿Òfý:'￶'êΕyÏ¿é2IÉw­·?ÉGŽAAGNbcuCRATES J081705+195836?ï™ÊGüæ? âÍÞþO<?I›Ûþ¼?=p·¨v'?‡û´;½b¥? ãŒBHBó?ïÅù¡
£¤?vÝ·6%Á‡?QE"Uä?W€ ù./‹?x±Ï/z"g?r¯È|Õlo?ïAS8?')í>{H?tÀ‡ p?~üo2ƒ?˜±nVÝ¢×?Žƒ+hðv¤?îëCƒ@~?|HlºÅ6¡?smePò¨?Xî×ïÙ­?¼6N1–?zÆñnÖ?ïƒécRØ?"É»Æ?`¥ñ²Ý|æ?W¤ê"`°?ŠÜ*ÍXïÎ?'ÍŠ{³C~?ïUÜ5Óÿú?'4.ZÜD?a²ØÍ¥°?l‹ÐÕ±R?"0)®ô?³Ó±·Ui?î"ôÐ,Ü?"¨Xá¹?yž`œû¦?~k-ìf‹ö?£ŒëÈPìK?'¹iÙèˆ"?í?6î ÿ?"ÆÄ "Z?ƒPôÎÄTË?t-1À-3j?³™×¬úŸn?"5ôIy­AGN4FGL J0817.8+3243?â'êñÙ@?{y¦µÀ:¯*‰@†À<pê?«ç@ a1R]oó?ý@"Êý¿´?Ï:N°g;x?Èü†c[ïë?ûòˆcp'?ûnºÖ*C ?ïgI}!"¿à–ØŸ8¿Ëñ†ÕòV¿Øx$>x¶ ¿à'¨9p¿éØæZgAGNbll2FGL J0817.9+3238RX J0817.9+3243?ïŽÏ¢û?{"EMWBÒ?[ßó•˜i?L>ûµºÙÓ?ˆé|é‡.?y®"åèß ?ï8Œºªƒ?­ž…Òíl?|"ä/æ´Â?~gáـçª?'åÄÿô£s?†~½]3°Þ?ï0Ó=ewd?†Â(ëõ÷?w@g(ÏM?{ƒÅùE:?"~‡éo¥?€.ÕW©?ì'l—?‰œ‡1M…
?—å¶-]?që…Ê"Èý?µs[—æê?‡ÄÌ)7& ?ï
(p{W?r((¢'e?p
0C©?aËÓ«HТ?š«nêT®>?NyŒhA?íë‹m ±*?¥¼PèJ¸¨?'e…(Ñä?"²']"Û?¨"gàÌÏu?Ÿœ"ð(?î>ÛÍƜÝ?™$Ód£V?…Q/r‰_e?…–'®¡'Ö?¦½÷FóY?"S¸÷žV?èèHíôT?Ÿ_¥¨®ë?¥-«ŒoÁW?Ž&^Q&á?ʤóùÑ+›?¼4[²ÃAGN4FGL J0817.8-0934?é_ÞEO²@,¥hÍJ¡À9÷І•±À;¾Ñ"Âr@«è¦
?þB>ƒÉM¼?°	ü-7›£?Àñœdûi@/ô÷í@	[wÿ@"?Í 18\<í¿Ø¢°=w/¿Ø8}%Ō¿â<a_–h¿ä|PKߧ¿æ"z~K_zAGNbll3FGL J0817.8-0935TXS 0815-094?ï¾\ÄH'6?v¿ÁÎÒn?^ØqLô§i?XTÝÒف;?yvœC_?t(Íô&k?ï'›'[ü?£yÐäO™?%Žh»»º?"
ð½xŒ%?˜$HïŠ? êގHá#?îû­Š<Y?—1ä"ﯴ?Œ:…ëo'Í?ßÚbåç÷?'rÇ_ßëa?Œ"GcFo?íM7.o?ˆë <9?"ÕÂ=ƒ(?m«ÚÈ8'?° Óx!I³?"÷?0$\—?ïNëËj¢?•í¾YÎo¾?x$'äïh?rÌ®Ò5vj?–퐨Uà?"›~«i–@?í8rŠ½?²Ù«Bé}•?˜B€­d?žUY4
?°."MÎk¾?¯ü‡5Ð?íÓÀþ§)>?¡ØÝáá?œ6k‹ â?–"ÈB{/?¤¨ºM2&³?š8©æ?êVŸP¸&?Ÿ¶R$ÑK?¢û¨<֒L?'؆ßiõ?Á昰?žƒãW†WPAGN4FGL J0818.2+4222¿å/[žtl@@²`˜À7µx!yÍKÀ;lðå°Éa@'ä6>U?ÿïCZD?–µc›þ?µ@j~N¬@ ­¸d"@V{Šæ¿ÄB1¨Ä"Õ¿Ú$¡4˜Ž¿â[Ã?…Q
¿áçø¢=­¿åŠK1Þt¿é3
ƒç€­AGNbll3FGL J0818.2+4223S4 0814+42?ï·_…6F?¬®Šïí>?\ÍNMhÃ?"¯ïâʑ¾?})'2ê¦?§µéš7ú?ï"``¤Û?£'…'ÌVø?yíY×,7D?QñºB´?•8v
,Û? _ç1­/?©Á]?Ç¬ìK?|;ۀø@¢?ˆY	kŸ??zêOÿ­?€Ü¥™äa?ïK¿vxn?z}C$Õeå?{eçÍó€?gwx"cŽ?Šou§Î›?sEí€ï?ﱆðA'?®K'"‡(#?[فÀ!×5?ŠäÿË1)3?€#¬t×?§µ¢$U?íτ§ïó˜?´¶ñb;0?'Êâ£	9?£d7"éL!?ª"D,Ÿâ?¯ÖÒ2‡ÿ£?ï–å]?‹#ž‹]ü?uÜ+9"¡7?ƒ")ª,;®?~±&XMVÇ?åfQ¼á?îgбˆÎ›?'¦Â›Zç?‹ã½Ìv2.?{<k#3??¢Šu1pÀ?±KžÇ¨AGN4FGL J0818.4+2816?î­1ó(gc@>là¨KäÀ:ªp-…DÀ<‡ËCòž@šÞ‡	t?ÿø€¯½È?Æ3©Ðži?Áío"3,?ûÂùå3Ì@5½'"Aç?ïÿqÐ&ôa¿ÔÆÆ"Ž ¿Ç¦F{9‡5¿ç骾…m¿Ó÷V
RÎڿ㟟m1AGNbllGB6 J0818+2813?ï·)^Àw ?'ícë>×F?CW÷â_Z?=•ê?(׫N?'Œ-Y–?ïÒ93äo<?mH•¯¤ÿÆ?H •
Ž…\?M¤!җÆ?sßSTÁCq?h²O©þš?ï!º†Ï?Ôàx˜pŽ?]¿v®û.?csî½¢]?šL¿vM?—¨Hvô?Юiñ?f›$-c¿Þ?`ÂÙttè?E–MÏENƒ?ˆ«†¾ºT?e€û7û6E?ïj=x±lŸ?‹§›xŒ{?XþF1·L?Q?[U2W?'(l€'Ô²?ŠçAÄi©?ï"8šéÀ?…é0ÍÖ¡³?YKyñøœ/?a
¦b"ù\?‹ÈˆÙþš—?"
äk"?î]¦x¶[?›7Áát?f®*F6Ý?h·ÉÄc®?¨Ïj·³ÿÚ?šÈtA~!.?î®á¾»*þ?†v'½é@\?r%šo'?b…?P•F?¢Í0ÐÑj÷?…¸Á4å¦=AGN4FGL J0818.7+3153¿Ø7ÝÆø«@?vq%Ý	[À;]r{ÛCÀ<´°X"@½ˆÍC•+@‹t"Ì?Ðԍ çìŽ?´˜û(·¯?悬î
46@
½©y
­Ù?î9Xç!â©¿ëL´,j?ڒ1%;ù«¿âg‹_D36¿ã÷÷ˆb9±¿ïÿæ¦SfAGNbllB2 0815+32?ïñ£0ú§Y?S¿ƒjÒã?*§…pdèr?!nTè?Yd­uaà?R,±î:?ïÈê™Þ°F?}`I¡Ë Š?O}g˜.À?]…XòBþ±?w©ÃpH5¦?y¿œyê?ï]u×Ñd?‰äe6?Y°¬Ø&!q?i'¨qÍD?'¶:7
\?ˆoÓh"Ç?ïµ,1-ÁÒ?b•uPñ«p?EªË?3)Œ²7R=?ZSu­]?aÑýÓè?ïÜò^צÅ?fØø¦°³†?8ÆNu²Hb?0"gñ(Ù¥?oô×>Õý?eë+Næ­?ï|j.ûs²?•ŠRýôz?Vv-M$ÿÉ?f‡¾³µ?Ž®¢}3?"#Ë]Í?Ø?î"À#qP?œT&Î‡?\¬¸_tè?c¤_«l@ú?¦Î˜5wX?œ?
p¦½6?ï%ʓÑGu?"†î‡ŒÅ®?UÃ}ïH:•?O‰*ËÈë°?™êu¦¶'Ã?":;@m
tAGN4FGL J0818.8+3229?ҕœ}f@?žbÜn*€À;.'4ùÀ<b¸®1×@Áœ/ñ	@!"U…?×Â$g¾U;?ÁώÞ§«?ð4Ä}ròf@«Ð9h×Z?ïÀ«÷j/I¿ãÓîÿý{Á¿éq®~-,‰¿à°!/ûpN¿ç&[L
¿ïíp±C‹AGNfsrqRX J0818.9+3227?îTÿ—$?Ç·Ûpv0?¥²3?ÇûÜ…~?†µuâ*æ?{DÁ¢Ô?ï|YǂÇ?†jóųH¯?k}/õæ‡?pðp´&Çm?Š˜'‰?€×ÄèžÚ·?ï)tn–³?ŠfÊ2¤?^bïVÄÇ?bó€UX?˜ëCID±O?'¾omÊ?îËóÇ@#?¨MʌÎT?oÔ´¢‰i?T0ªëò?¡CxB	yv?gÐÒ ‹M?î…W,YÇ?·Jõ4\ ?—'«ë€Â?·Bf9Tf]?˜-n‡£÷?h#7ºí?îÞã%Ç?›1‡Þâø?qá!ÉK‰{?yfَ¶@‹?Ÿ«UW'¿?—ñ°_ms­?î\5Œ(£?›6ðåäT?iex¾¤^M?hºo²tÅ?¨¦O°M'm?š†U·EÏ?ì&piköÁ?ŸÙ´ð?Ì&?€h»ò•¤?t{÷1¤6±?¼¿yýò߆? nՀ›=AGN4FGL J0819.0+2746?î|LÚ-Í@>j;šàÁvÀ:v[ËرÀ<y¿¼CÎ@‡ފºY?ÿ'è_ÐJ0?ÉIøÜö¼?Ä`EKc¬?ý&ðš1o?þ¿Ý/ñ?ïùï2b¿ä´Ø"óÙ¿ãã9Ü>Z¿×Nø 7­ì¿èLˊ­n¿ïÿÛLÂPrAGNbll3FGL J0818.8+27515C 07.119?ï|}ˆ'<–?IbÏùí?iQÕ҆R?^ùˆÔ±e?Š›	qðú?~£Ãl8{ß?ï0co?'ë/L8?€óý´êa—?@¥DÇ'?"¿ô¿]?‰Æ9¢ÈsJ?ï+ûZm£‹?…€p'Û;P?t

¿˜>?tã'ü—?•~Aµ›È?'Հ?í|ÿ\c{?†þùMfîª? s'^fè—?zD݉A_?§Ê­¨cCÄ?€ ïø—Ÿ"?îõ¿Ký%ý?'ôXöÉòé?yV£K±E¾?qÂ(í<·?šòm¨÷pê?ـåBº?íÏm'¦?§g/³"¶÷?"[äqy?•áøÒû?¨â÷"AX?ŸøZÞâ'Ì?îO˜Vx‡¦?"›È'^">?'D{!aä?|Ö,Ut)á?¦u[ÑÖڔ?'p奞¦?ê2‰±Úû?™ 6§?°Ò_Žfý¾?"u‡c¦?½™WÕTå?–0[ndtAGN4FGL J0819.4-0756¿Ô''ÿ¾´@.úò¥µ1À:¸—/\À<igÏòñû@!™9ÍV5?ý?cr–'?ÄG?D8"?ûžû?Íi²KAG?í°T¸'×¥?ï³~è=k›¿é°iS¿å XóÖ&¿Óˆ!Äuæ¿ÖM
ú¿yR¿Ý¹žrAGNbll2FGL J0819.6-0803RX J0819.2-0756?ïRxÂŞ?°Ì2•uë?VVøTþ?ODHë2·?"SŸ›XŽ÷?ŒÚ×IY?í©YDÓ?·¼•"¼?ˆ›Eà?‹%!§¹z²?´ÉD.ûc?¶¹~"#z?îÝöó¼Ð«?LÐoÁ?t;õˆœ€?yw>ú^yâ?Ÿ2$#ý‰y?‹–Ѳš?ëZ¸èê9Å?˜UÍÓ7>?'[ξܢ—?uõl‡Ìjb?ÀI¢'ö›?—¨
 —æ?îV°N?¢yÑfO^?h6úó­Ð?b @²¹¯p?©Ž™‰Ÿ?¢°AÂ;P?èú¸½÷?Ê•æÂÓ`?&RÃÞ?¡èмq?ÌKMR»† ?ɂ3v
?íq¤iùG?Ÿ4_ˆDÀK?'ÂmtãÜÓ?…s'~™ïó?²Ön?œ¼ÂF>±I?ä0¯‹&?¬Ôý>âÎ?¤æŽ]í?'AÁ£¥4?Õ 1‰öõ?­æÏ'ªAGN4FGL J0819.4+4035¿ÐºÜ?0—x@@­UÅ.rÚÀ;ZÄ"ðÀ<ÀëóÁ{@ xE×Ћô?þ©Úª!¨?ÌÕ2÷Ï
?±:‰hÉíõ?áDø®ÖÃ@<pŸû2'¿ízÝð,¿âBMb3{Ø¿Þl~Q¿Í¹±<"›¿æ²"L*zþ¿Ý1a¥1'AGNbllGB6 J0819+4037?ïìzH¬9?I܌x,P ?3L yñmº?î݊"Uà?ahlÙ"Ã?HƒË
Y½?ïÊ®€?rԀ™;¤?KgñÛÆ?QZ%­éþ¦?w(r¸ÍÈ?p¡òç:L²?ï+ï–?oͅk¦¢…?YÃrÃ?AÚONN?ˆü•ûF?n(̔õÜ?ï‰Iê?f±¢®yþ.?YäÆrN~Ï?=ÎÒö6LP?Š'"«"cä?eä7;íÔ?ïÝž	°?^…~¹L@?>˺W«§d?/]ÿñ÷?oìˆâç?\ËñÄt¬Ú?ïk°¡.I¦?ŠZŸ,p?Z²j'Ì?b'«ýŠ?è€Áã8?ˆ#GžHV»?ï8ùk	?}'š±¨œ?cŒu{Є?YÊpú݌ÿ?–~ëˆó°Ç?{zt©_áB?ù8?…¤Ì?ÖA?oé]žŸ?]§	[ØÊ°?¤•Žë<då?…HVNùßÁAGN4FGL J0820.1-2801¿íöKêAÛJ@ä—t%kÊÀ;nE£x?­À<ŽOËð-û@#'Òëò_?öø¼ßï¿@?Ñúj>ã¸?ɒOù<—`?÷—%¶rî4@á)`Ìt¿ïÿþÐñ?ïþ!xöŒ¿ïÿã_¶Hý?ïÿð`OËð¿ä2M?Mó©?ÁcÄÄÂAGNbcu1RXS J082021.9-280206?éˆÔ
o"?Çîý(»O?g%aaºr<?e«BÁ¢‹?ɀCÅt
?Çܬ~ßÀ?éÿü5V?Æ3o÷½?­±ç̅?ŠzÞ{tï?ʒpX'£?ő¬"ŒÙ1?ê]3²è}¶?«s$¯ Æ?€ô4…nŀ?¨âë§ÃP?Å{íê²C'?ªÜÜ:[Í?Øá?˜–5!z+?x·£ä®èL?rë_vh€2?ªð WHk?—¿¿ÇKq?æ¢Jlå‡?È
éLé?wQ"agI?w]íµgbà?Ò_YžÏ/ö?È?›» Â?â§?ڋ|J?λŸ¼&?'-¸É*m÷?²Ó°µ¢¶9?َ¤¾:ã¬?Í£]²ã—•?èL˜H
?¬ébeÃÛ?ˆ
]ëÖmÙ?†uáZWÍ7?ÍN»¾¡T¾?¬€ùñT
?ê3Ÿ
-À?¶!©"î¡ú?™}ŸÜâk0?ŸÞØa,J?ÄÏÝg=–?³™]%ùM"AGN4FGL J0820.3+3639¿îeìzßf¥@@l% Jù#À:,Ú"ö¥
À<uo·HJ@Š%»üE
@"€Þô?¶èô˙q?¤Òhÿ./$?îRœàKß@½½"J¥@¿Ïœ¤ç€'¿áÁ÷Tð¿åùéÀÎfÖ¿áyPFGã¿ånbHÊt-¿ç!ñ¢DõAGNbll3FGL J0820.4+3640MG2 J082018+3640?ïÏiœü¥ƒ?`ºð\™?Qt)O?<4¯1ßoO?sύ~#¸"?]Á*.5•?ïÈ6™™'?uÀx˜§ˆ?P^
®ûó?W:"«‹â‰?wÁ%CÅHg?qŒ¥å_DN?ï€j
àˆ?t'EaYœ_?b´Ã çX?M>Œ®Í÷?‹8K¬îäc?rw9àZú÷?ïb7ëÝ;ã?h°Úbˆ:?w~üáò¶²?SY—#/H…?‹²†"HÓ?eR52åü?ïŒVïT?x<v輄è?cÐ`%Ì)?RW#@ŒŽ?‡ì9ê?uŠ
ó–!?ï]s@>‰~?Ëªwˆ-Ô?dßî-í¾}?o{ŸþRÎ?'µš7@Œw?‰
œ[ØÓG?î赟oؑ?Š+@íÓO?rê~]ø«?f»•óìÔ?ž.¬ƒ¿£?ˆ!PúíÄ?î-.Ž€-Y?‰Ñ²9΂Ú?'"O½'tU?sëÄ?fƒ?¤co8‰B?†ø",˙AGN4FGL J0820.9+2353?"ÐñÝ8@=ŸÑx-8GÀ:ÎQ1JüÀ<yôÆ)@¬K&ÄåÎ@l#ú±¦?¼¨ñPdÇU¿²†æ¹‡÷?ô?I)>¾@5."hƒ¿åñ¡mx~¿èOÄÎщ˿äÐà,Ðî¿ã ÷&<ª«¿àWg€桿Λq ?[AGNbllGB6 J0820+2353?ï¹ÂÙ?˜ðpƒ]±?U.¡}‡K?o?©`Ó~¿?~'òÔpŸ˜?••ÅÖÛ?ïÅfß]<?ss~É|êÆ?J¾OÝÒ®ø?PN5CE™?yôÆP²Ñ?qL

–(?ï|ÀUM?w×¼c?`;L>Âg?G¨Z!§1?Œðüå•ÜÑ?v@3®ÑŒÂ?ïšê1a¡Ü?e¹³å}!Y?[»Ü$þç?AGxfûV?…Íø'
ßA?e·JžM¢9?ï|Y"'?}¶Ñþ"é«?bŽðÅÏ¢?P³g™iåv?ŒEÿ^\',?{۔÷*'Í?ïUÌ'îå?Ž;%üÜš?`GhIô¢?f+/Ù?"=‰l]Ö?‹Æ*/46?îàDÉçã?Šm…ýKû?p)Ò1ž²*?gæ/~B?Ÿìò=;ù?ˆ=HÃV‡?î"+ˆfbØ?‡µ{'?wt¼ÇôYY?dùtr.í?£Þ¯á8V?‡ë'jpÛAGN4FGL J0820.9-1258¿íGàRÕSÉ@*X©XS~,À:z:iˆYÖÀ<^ߘk¥@֊þÌ#Z@ɀ¤Ö
¾?¿3~݀¤? ÅoôZ?âObcøM?üû@}ž'?ï×.Ož£Å¿àA0íÕ·¿ä%"S·79¿ã%aE•6¿ÝrqÂ:!º¿ïûOyxAGNbll3FGL J0820.9-1258PKS 0818-128?îßn¤gAÇ?ˆ®Ôƒ_?iRcûT+?W÷:.Þ
Š? sï{xqV?Ðýo=5Ò?íÊÖAY€i?²©?'ÖÑ?€%ÝH"Â=?'áZŒLW?¯I$™äÙc?±¦ÙEÔ?îÝ	ÛB}Ë?‹ÎF,[¾ó?uŒÉzÓré?mΧᏋQ?žû'>"ÓÔ?ŠŽõ^ë?î,Ü $•?C¯™>Œ¤?ˆ6ÕÏáÇ?h$–Ï›!?§1hM‰Z8?~}v!i7?íg¹‡B ƒ?¥bmàè"}?'‡ÄèLd?u%ùÑäv?²€bÌ¢Z?¤?õ2þw?êAa–•Oª?ÄÂ0†Û{ç?¨ÓðÃÒ?"ng¹8 ?Äÿìgzk4?ÄZ…ƒHZž?í4äÓv+£?¢…r/p§?†ªà:~0?yë#Vëû?³–"GS$?¡bꓮ´c?êà3'Ó?™
$õŒì? X5¡rl?†ãÐ'?Ài¨£€UÙ?–ir¿£	(AGN4FGL J0821.1+1007?ï_RÝá@8~»˜Çâ'À:ʺ?+ŽúÀ<‡Q\&M@4êÕeM@…ôäC?ÀxD_U{¿£*RŽîù?â†i`Á¶Ä@
SÉÇߨ¿Þíӄø¿åSŠS«y¿èœ!3Vo¿ß[º9¿ä¢aôçž	¿Ú|=&|AGNbcuSDSS J082054.81+100609.4?ïúŒ‰ÌÙ?4Bø˜×0?#æ=w­l?qKM;?@ÔI@'Py?1lîÛ¿?ïç¢íf†ƒ?ix'HY?7ÜKµßÌì?F;»oT'Œ?ea‰;4Tã?eŠýá!o?ïÆÖ*¢?c¼ÕìÚ¬?P*$£'úë?7ÛÁŸyÓ?x½h?bjÙh±H?ïí6Ý{Š??pW'}ˆ?6ï¶tÊ´?hb긧?`*ªþ7Õ7?=´Y¿‰R?ïø'mú{Ô?B6>¡$0Õ?-"h³"ú? 7ûÔA¡?H®Z‹d?@1ÉצÚ?ï¸-C6›?Þ9—‡?Då½*=?RÁ´yô›?€²°ØÙ­&?€Ä¼{ÿ|c?ïf'¥"?zõÇJŠp?[n5¡zI)?W~èY"y?ˆ¸¸ààÌ?xOk¹¼u?ïÄÿÅ?a™X®Ü¦?Q½ ï#7â?>–n‡Š?y+Æ2Kþ?`N00¿¦wAGN4FGL J0822.4-2630¿Î:¢™®£}@ãS÷ÎÙÀ;
1'rƒ«À<_")P@0<yûš@uØå	µ?Êúv=Éå?µù…½n¶?îÈ.ØZŸ‰@kk!ŒÏ¿Û½*,ú4?ïïÙAOU©¿ìaÏþ°t§¿ÑHdà
—¿å!){#ŒÍ¿ïÿÐ/WÜ`AGNbcuNVSS J082236-263125?ìý³Ì˜?«€o±P¶?f¬Éþån?\›Á`;¹?·a´5]L:?ªÅMYR–K?ët
Zï1H?ºI†[Ï4?oîáb³¾?ru¸%7Rk?Á°+ðQ?¹pÛ¹%…^?í,袰‰?Ÿm֏q·"?—§Âu\®?tó)Bò€?´Ÿ@n!t.?uEÞM×
?îö×Z3A?wÁl͂Ý?yù	ô"	Á?]VgFy?šÁ¢"mtr?u‡Éƒ.W³?é{› ¤²Ÿ?¹à¼vpþ#?yv4h¢?q»H‡Ú‡§?ÉEáØïè'?¹«Û2¹ï?åBð;։©?ÇP"Ö0N?…×ÓºG|%?•wžsÓIY?ÔË`ê.:.?ÆE±xf Ï?éy> ­<Â?ªÞ+àQ»"?Ž‹N~óbÿ?ƒ',¯€t¦?È2P"íãH?ª*Ëk÷4?í4ÖHC3?'´£´pL©?«®|Ò#ÿ?zÉ>3לÙ?².b×Vi?îc(!÷AGN4FGL J0823.1-6330?ͨáñ;À-Y± žÛùÀ;¤öL"'À<¿';ý@"Ùa…«ü?úaAcwž?Òæ">eìC?°=˶¶¶?Ý¡faÞÂC?ý¤¬	ˆ¿Ø¿ïǃý{u¿èó.0D?æ/ùø??¾îê.£ˆ¿é²ò€»|B?Ùã&2ƒAGNbll1RXS J082316.0-632928?ïÄç80?Œ€ç"nÿŠ?7f€ëÐÉü?8¾J]$?|ûäð3Ÿ?Œ:žqhÐ?ï{"|w?›–1knR?Y}˜±;ž?dNÌ8D?Ž¿\¹ÎÊ?š`¿ý>V=?ïB@2[X'?…=ý3u?dvØD"J?nùÉïO?•7ªÒ5­?ƒ:ò‰½¶?îÏ»¯™
?'"–ðd·?W3b"0	n?F±ó<ŒÃ?¢Uy1®ÉŽ?':x傚á?ãÁÓ?‡(ïÒâñ?C4ÎpV¾½?6óìMø$ò?ŒÈJ&׿¡?†òìº}ë?îù¨-cÃý?©Ž½ÿq¾?cVë†
Å{?vµºeWÏË?ž`åæ¤?©Uá6zá)?îԃC°±?ËåKgÀ*?híä‡Ç?m'·ŸÒå?¡6lêFû?ŽŽbÒ¬?ì³>0gPò?ŸßH
Öe?fÃYQò
?cá;ù'5!?¹± a	a?ŸàH»ÁÈÉAGN4FGL J0823.1+4042¿ÐçéçBw|@A
CނØÀ:K _ŠÀ<S½—¥£"@E§håÎ@Ľý&0ì?¸ÛÖÕå$]¿˜Ù·–Ú¢?ßi›"Ö>@KÖWºüì?ê_ëä¿è°Ô^;Ÿ"¿æ†Û†£ó¿çÞavؤ¿ÒB&€IR¿ïü5ۄµAGNfsrq3FGL J0822.9+4041B3 0819+408?ïØ>Ȓ«i?«S⶷?9NΈ`C?1ì3?Óh?rK®Ë<Ò?«UëT±ƒ?ïæÜ;p•?l<ÆÚqï?8Õögs«?Dïµô{?f	
DuP?hqNÇòF&?ïŒZÀڕ?'¦š"3TŽ?SÍùÉ?>kG)æ/?ŠœWA¸å˜?'›Ï†ü?ïí¶ȋ—?Bæ¯ûíÎ?,#¹kÄmŽ?ÅïÈgÛi?`‡®¾!–Ü?B°ý­pVo?ïáSñ*
|?i5]¢x?L0½FÂp?Cí±¹>E?gŸßšŒ9?f¸I¯4Ú'?ï´ÄèÒ¼Ñ?"‹ÐăF)?HÛðeöW?Xڕ`ò'˜?A_gãw?ƒW³˜bÕÀ?ï%:MêÖ?Ž2AÃ/DZ?_øÎÑë`?Q+(qk?™n¹'E—?ú7ËÞ?ïÂlv Æ4?cùž‹Œ2?J"`.?9^¶›¿Wÿ?{†ÒEbé?cMWÿÌВAGN4FGL J0823.3+2224?îÒÇçF@=­gf@¦¹À:q(•J€À<rv.Z†^@yðÿ±üg@#Nƒñ'¨?Á±=òÕ?º"»¼Pí?ö4ƒzsc¥@q,/³ÌÌ?ïªì¨4g¿Æèž9'q¿åèº3mÖ¿å*@ ¯¿ã5ækÚ¿ïÿàŠï²«AGNbllOJ 233??yØw"_?^ÒþĆw<?Rz.‰q(š?ƒžva&ÿ¨?wŒ"xÊx~?ï¹´W=²?vÌ¥Iúï¦?YláAÞM§?^wl§Täz?|ʜ	 ;:?q…˜‹"0?ïgˆöðH
?yÏî)eÂc?j"i6Iòù?dZž«€²?xçñŒ÷?t·7ðu^'?ï4DìªHû?omáWÞ+?"6êÎn¦:?cC¼œ5Ó?Ž·Ú÷9(?eÓöAzE¯?ï6"U£?ˆeŠ÷©ë?qZ.p;}?c¹ÀóQ#:?"å3~1o?…g¡ŒÈžì?ïB™wà·:?ÍdУÁÈ?nfö™ æ;?t®u—Þbß?"ßò5Àjå?‹°Ó&kD?î¬äåûÐy?ð¬Nü?€]ÔC|2?x썊8Ý?¡<'
¦_?‰'~Ã+B·?íâÍ(¬
y?‡…ÐFÑa?™º4*YK?€ý´gxz?¤ö`7«Æ?å}I4,ÿAGN4FGL J0823.7-4838?ÎÞé~xÜÀ¤B"ßÎ1À9GÙ.ÚÞÞÀ;-‡É},@'¶iÞì@uò£ +?ÀAž0O‹?±j¿ë½Ô?ñj µ'-l@ÛW‰Ôª'?ëGU^×%ì¿éfA·/'¿è¦¶~¡Ç¿åýÃÝéU¿ìÔ
xÿÆ¿ïù·KAGNbcu3FGL J0823.6-4838PMN J0823-4837?ì»E÷2?´}P5«B?|I°oѺ?tõδ:¨?¸a<ô¼¥Ä?³ö>-¤Œ?è>gÉÔ*?¿ ÿê[~?'ô8Ër_'?"=M°è`Á?Í×N«šß?¾|®Qaœ}?êƈ°@?©ËìØÿâ®?˜«?-ß?'FZŠîŽœ?ÁÒe×¹ÿ"?§R8_'?ëVb
6:?˜ f¹Þ¸§?–~'ò?rØV6?¿È P鍴?—Á¬››?憃V%{?Ãh­úŠÜN?—%4w=ê•?'ì­kG?р¦]u@?Ã6-Zùm?àJÖȤ-?ǔÄíf~?–±.ҝ?§µÕ@æ×?Ýÿ?±V¶?ǂ#6Íâ?äYT}ŽSÉ?³Jë•ø–?­âM±qy?œ7kj÷?Ó©Z»Ò~?±B"PZ?äÏ"y?ªΰr´?¯9èO'?'IÜön?ÒzÕ{>‡?©ðkfÙ½AGN4FGL J0824.4+2440¿àŒ.Á"cq@>¢v§&JÀ9žØ:¿¯À<û¶Å#‹@k"+'s@qý"ÕíÞ?°¢"hR#ä¿¢…>©€d?ðÑ}†=œC@!BԐæm?Âcþ"8¿åâX"ÖÅ¿çñâÀÿäý¿áÆýX…Ó¿ç¹û~»òµ¿äGDžkAGNfsrq3FGL J0824.1+2434B2 0821+24?ïûã?ÕÙ?.M
•¸°o?#ðcçÐþ?s
!¢O?=³aã-?)zª[ᗅ?ïé­ÕTŸƒ?g¬K_?5)<¤HÄ?B[QÇx¶w?c­ÿz#Q?dL^á5'?ïÀõì´Q^?h·œržL?S_õfO'w?>Ç߉:?z­Aô˜v?gƒe™?2?ïø'_{¡È?1R⧀v?"`'Þ°	v?L¨ÜÕó?JÊ\"ø'?0®h?"åf?ïù0Õ#Í)?94âò4¬?-|Ox…½Z?‹Ñ_®n?CݘTm?5Í@"¸y?l֛5Y?‰Qû0ž"'?HLqC£ó?XÒdP^€?~0È!ªê?ˆlLD×>y?ïÂñVÄÞ?yæ*Å:,-?`
4®ªÅ2?X¤)]!]?ˆŒ¶{4{H?x^}¦w?ïè~Œ"Å?RJUÍ4³??e€ÄdpÄ?,¥:¯"AY?c"Ý®d?Pˌ¶RQ"AGN4FGL J0824.7+5552?Ä­"êžC@AüPHÀ9yú Âî'À<b[ŒÐ×@ŽWáé>@ÀY+",?ªæ%®¨?ž½»"GoM?î\fhå@͘îxîÿ?³ÜÝf"â¿å˜ËЮڿç»ÉÚª"¿èœm¿ ;à¿å(œ×;»˜¿ïÿ±'#áAGNfsrq3FGL J0824.9+5551OJ 535?ïõŽwýh?rT‡˜"î?/$™'"°?BPmŽ±?QöOŕ–ð?pï+Ùæþ_?ïäƒ-$.?hڄÖtŽ?=W—
`?FŠÓ¹?gÚ'Ú^¸¢?e!LèNP ?ï¼q,èì=?mèaô«ÔÖ?Vr±-v?UM85Z8³?|FÌä½ãà?làSJ&€?ïø?ïP§°?22ŠÍçÃ?8g¨PÛ«ˆ?!_Ø[iÇ?BÌn®Ê
?+	Bn´áà?ïð¥ê]p?afÐ|®I#?4II²+rK?@[tmb
?Y¡Ùdxæ?]•>·¾ý:?ï²3ˆºñz?lܨU«?N¶ÄÐß¹)?\‰u%H?‡±‡pzþ?¹"
X?¼Çñò?ò6fv?aþ§xï?]WçåXg?ŠT.ŽyN?}\«/£Æ–?ïé׿;Œ?S#1z¤Ëw?Sˆ °¶­?Dhin#?XÇá\")?HÆ_3—½ñAGN4FGL J0824.9+3915?ï÷®LÕ`@A¦ÊıÀ9'ÛçòÃÀ<Q¶¯T@ü¦–WDà@öƉ¼­?±Ï	¤ïc?º@ÂèÈUð@fhÝ9+›@˜q±CÞ?î¤vlmçd¿ÝM'iÒ,¿ç–ŸV¿äq¦ ¿ç¿ëÙ~áÝU0¿ïÿÏù§÷*AGNfsrq3FGL J0824.9+39164C +39.23?ïÓzNá˞?p֟%?SVÒ©>þ?PϘ>Ð?qm$ ý?j³Å"·ž?ñÛ¥?Œû·°€ÇÙ?p1yÆ#h?zŸÛ‰Ê_Ý?…üÀ¼eyì?ƒñèNB?ï†ÃÖ{o?†<ì¢&?vŽï€TD?€¡²i·?ƒ7 ú3?z'NÕѲS?ïk!ã™[Ë?p­*Pyª½?ˆÈÐ$+i¡?kWš±3'?xÝmØmc_?YÆ헢
{?ï…k$«?†!/n<?iߌh·?azÏ?ˆ-Y5Üä?"-H£âç¤?îå̛'/£?£ïškÌbâ?ƒYy÷Èc?–ùð!&?™™¯'9?—'GW'e<?ï2Áƒöø£?‹I8±‹ù?{æùýê…?€¨ë›ñA?'®âz?…gÙ½|÷?îeM5¬£ü?Œáþöå®?¡£EǍÝI?‰´Ñ*Ž?Í»OÅè?tQÔ¼ØGAGN4FGL J0825.8+0309?ÑFàM¡ã.@6c¾˜V£{À9‹¶–ç8À<>æ¾æZ=@쮪ì}@œ@WV?¯_8ÕX7¿@¢>ͨç?'i1qçú?ûA7ë~¾¢?ï7É
ûk¿äÙ¸£J"¿ãœ
!Áñ§¿ágFáúÊ¿ã‹= Êei¿ÙoÐ<ÃÕ­AGNbll3FGL J0826.0+0307PKS 0823+033?ï'[êâaŠ?RÝ·œŠ?^䦸±ý?P»8–Å5?‡æ¨¸gÝV?|è%'P?ïIÝÔA?'ªkx7ä?uÒ®Ý$h'?{á–hxØ?'O°£h¨Ë?‹`"Dî?îÃ¥r?žºò&E?"ç‡F'f?"-¥öæN?ªyãáZ[=?œô4
Ü^&?î¯Úa?'o‹zh¡?'u‡ ÛÄ?u]Á3?—,>ˆ?uu!ÀÉ!/?îó#¦M\)?–¯: -ë?u‰¡`½(?ié܅U?œ9"÷«çˆ?" Z4>	?î1³ŸTD?¥Üˆx&ZÇ?ˆýZ•?\?'í'ëi`?¦®¾or5? S²>õT?ísª
?¢òÃL?‰jšá>à?'‹©¤N2y?´ÚšQ
Ž?¡Ý 8'
q?ì˝bQý?œÛô†Dë&?§$/¼œ…?%¢luò?¬!úȬ?'ùÛ–YAGN4FGL J0825.9-3218?ç«P‹]Á§@
tO»)6ZÀ9NW±—½!À;¦€ç,¬@"­K¨@ºZÚA*?·ì
µÂÅ?Ï£Û¼Ô²@è&grÕà@wT©¥€X¿Ù߄ÊÕ{È¿à"b*—ƒ¿éE½úL¿è5QGq¿îÐîdÍ	3¿ëÓb}£™ÎAGNbcu3FGL J0825.8-3217PKS 0823-321?îZe³°i?³#œ‡ø–Ü?™Ô¦àÔì?§Þƒkuh?šçÌhµn?¤¾šÐ'®?îF՞ÏÜ?°
>zœ?r¯ݘEŠ?}vlC¤2b?¬%²£šŽ?®ºäÈ
(?îHק=¾t?š3¼¬š"?'ÐXLºq?Œ"ƒó?¢ŠxàÙ¢ˆ?"o
3fˆ?îÙë9I?x9èZz%‡?"EvxïÀ?c¸'
A§?šŸä	Êò?s€Lß?ìZ|EJâÒ?µ%¥I-Îù?¨É'Oõí ?¥#±O·±?°ÇŠ-?ÿ?¯ô¨Þþ?êOÀÇ}O?Ä·Mxrœ?ŽmÐÛ'Ã
?™%;qòÀå?ÄÚÓ|`Æ?Ã['×?ì?(>ô™?¨È|T^?¥Šã
‹P)?šïð¿ûk?³Bm7æÌ'?¢ÉÿxQ½?ìÜÝyuëG?"(|š0Y?ÿdþ¼œ?…%24G¿¹?±™PZÑ?ð4Øe7AGN4FGL J0825.9-2230?ßO֍ڍ@!ÙöD•[FÀ7ތXhvâÀ;J	{¸@Ô{Aê±?þŽ&žÐ:@?šN‹9•´?°…OŠ¬Á¿@ÿkã}é:@Í+Pæ¢a¿£ãŽZKP¿×ôsúù…è¿á¿6â]¿Û@êa2J¿äšÀá@¿åuÀ –ùVAGNbll3FGL J0825.9-2230PKS 0823-223?ï–e¿â¯?¬ý
Òé€é?H-KÉ÷?E?VáˆÃÍé?ˆãé–S‹e?¬S残žM?ï'óÉLú?'©ýITMX?XÑufQJ?a1èððɦ?Œ(ßäk¯?'	;7ðy?ï|§‹Ó;?†"®H3gº?gw±Îæ{?rí"êy+?Šø0"!©?"AAAÞ#?ï³">Ò}?díúØ…Ä?R³Õ<'qE?8-´
ö&?€àõÖ2à~?cÔìåÈ?ï^/5?†«쑚?Fˆ(xÓ|?=֕ºM`?"…Þãþ?†klç]<‰?îËjƌ/½?ª¡#´?l eÖŸã?yô*E	?¡M8Ô,?ª*`³–gW?ïiV}1¦c?‰µwæ-?p+ò¨?w¨± Z­½?"Üžæ…g?…½µlµ?ïhæ£/?{¥KìÏ	?aرJ¥ì"?QӃnÅ?¨lՔ'?zÅ6AGN4FGL J0826.4-6404¿Üó-äê¥ÑÀ-XçW'Ž
À:‡‡H^>À<='JSá@!ã~êì?üqšânõ?·SÈ)$?œ(b}VK?叀[@áäÃ
±D?ëEKß&–˜¿àȳÞq!¿Ò•½Áìõ¿ßû[O¿Ø¡ŸAÏ-O¿ÌŽ9G¡AGNbll3FGL J0826.3-6400SUMSS J082627-640414?ïÂ<Ég›"?yá°pâ÷u?BD Áú?9BZò'R?|™íó7?x¯ƒî'š?ïǜ;+òo?}yGEå¢?CÛ¡RRä¦?J=Ol´?y¶n5m˜/?||'0–&?ïs%•|)?~…R¢0?\›nlõM?RX*'M?£RÃã6?}ohM[Ot?îÿìÏ¡"c?uWç Ô8?cÇ$ÊkDÜ?Bö(Mö!?‰x¯vø?uxŽô?ïr}öI?ŒT$ši"X?X©/ÛX4ƒ?UOšCûéÙ?%ËGC–?ŠZÝAëÜ?ïpXBƒ«?"ßlU¡n»?[dAUÝ?z›ôc¦ÚÖ?K"kuP?'€–ÊVŸ?îÚ槮%?ÈËùL¹j?h"†f€L?ai‡ì'¢? ÏÜO5m+?Œm½ Fq?í/*²Ršy?'îæI—ðï?wïQ_*ÌI?a¤rˆW*Ë?µµWWƒ3?'ïX–XÂEAGN4FGL J0827.0-0708¿'}6F	Ã@1† yKÀ:¼gú»À<5m%H{@ ®TL2ˆ"?ú݁5ž?À1xÞc"9?Ãúr¢^å@7ßÖjÛ@ûEá`­•?ïòMZ%æD?Ýêßqêþç¿ÂÑå:Ü¿Ï÷ ÞFò®¿ã™:Ü¿ÖElÜ!SAGNbll3FGL J0827.2-0711PMN J0827-0708?ïÁj†º!'?næ` 4?aqL"ߝ?Wy³&àÍá?v'.ôe¿6?gëˆOËi}?ïœÀ¶Ðt?†Çщ"?g!7ö 	3?oÎ,dŠ2¼?ƒ"DzÒ?)kˆ3­?ïff܂øB?ƒ²æÆ?äJ?m>Œ%'^°?u´î½€?¥Ù¤é²?€OÒ©41?îËa?n@Èŝ®?Œy°ç[?hN,v¼$?¨µolÔ?8qŒ?…Ÿ;?{_6'":s?r–P`€ù?fûÈè+—ò?PSqÅ~Ë?uK¹Š?ïì¢fX
?œÑ¾5å¨?yR{༑î?'EE¯	¶ï?™-̼½¨E?–Í¥
5àœ?îÆΏ´WO?'¾,Û\/÷?t@µƲ?vÀ-ù¦?¡«¾?'pë+…àl?ëŠvAêu?—^uzW>h?›³ÖrÈ?'7¸ƒI?¼Âb™/ïå?•GŸb±®AGN4FGL J0827.6-3735?àrOßÚ?áß®PàÃÀ9\‰Õ×7ŠÀ;-«‰†&@ŒhF]0@ì["e…–?Ì,Ë:%•¼?Îñ¬€&+
@%[Új@
±´Ãk¥¿Á«w½{Ëþ¿å`=Wyc™¿ìD‡•¿ïýÜ¿‰k?âɃ¡àø¿ï¶1J$ç@AGNbcu1FGL J0827.9-3738PKS B0826-373?Èúk}?¡u(,6BF?d
£Ç¡?'"•cǀ(?'JStìó?œöՃ…?ë".ax|$?È"›?rÑäÁ7¦¶?Œ©©¢ŸSw?Á·R´z=?Ç¥z>pº9?é£Ï=ˆx?«÷ëÍÏô?£9zu$?˜b€7NÊ?Ä¢dni•?©RïôÆ?ï£]ißäú?v½ì<Ý3«?(pSà\Ò?#îqUa=?†ÆåŒt2¦?vÊ'ßÀ?ï5€â,tA?¡©gê``²?o9!=?z?Ÿ9;"?•m!NUä¾?ŸÃ€·<¸?èfìÒÀp?ÏC'3¢?{àûL	î?'õ΁`pa?͆/­JY?Î(;čtX?æ»ÕÃÉ÷?²©¥Qõ?±Ë.iAY‰?¥¥WóôéR?Ì.%uc?®û3󏓸?îŸë¸þÂF?šã@Á6"?PnôÑäéÃ?TÈVàÕJ?¥}Ì̆\Ï?™µê"žAGN4FGL J0827.8+5221¿ïÑËup@AÔîàóË>À;Sx›ó-À<¸[j‰á–@ ‡%["5.@µPy•T?̊›9ÖÚ¿Í¶ùôº?Àvþ#±àã@¿ñÇx?ëKå±  œ¿è	cr– ¿è]ÕÉ ¿Úm¾I|K¿ß[ÿDÄ*<¿à]¾÷÷ôAGNfsrq3FGL J0828.5+5217TXS 0824+524?ï̸%±üx?l2¥‹–©×?DÞc›þ•i?5<ßÇÚü‡?w Á.ɘ?j–(€'²³?'P?°µ…‹e?efý†oB?jËiKÑ@?Šy€eNW?ŽÇHNYq?ï_þ]=Å?€åú܄Į?a:ŠŸ¦G?b¶ö˜ÃpÜ?'ØâýI˜?ä&7¦¥;?ïW®ù¹P)?vö>´p¡?aGÞÙo=•?D@ϼÌï?'á$ñǛ?w(Wû¨!.?ïv劼d¨?‡±²ÃuÜ?S±Œm?Jž>Qê­?ãú.èr[?†&`ìóÁ€?îçÐÞ¡­Ý? A*ho'D?p=æPe¢ä?yrȹ0§?žöj'ág»?uÖ~£àJ?îÃ7ÿ†Š?Ž$./(½?dþ§4<À¡?RˆDu[?¢|•'rØ?k>ÿÆÔ?í~•ø'æ­?˜ù†?ÿÝ6?z­álˆŽ?k5?é)BÒ?²`r"à"P?™¸ƒöŒgAAGN4FGL J0828.0+2307?ï×z()@>ﯷéÀ;
ê0ŠâGÀ<Ÿ	"5"@ ü¢¥‹•?üÉJç"Þ÷?Çö·ÂN™–?¸'ˆá±O?ñØyÞé/@~ç­Î¯Ñ¿™ª8€Ø‹%?í¨ÊߌÂò¿Ø•Þ#6eî¿âHdóŸŸm¿ÉÞ¶Ö:µ¿ê³
¹—eãAGNbllNVSS J082801+231215?ïÓã4^Á?btí§]³'?AkDaD
ý?2:EErú%?sàýK'Ä#?a[$eÓU?ï¼ØÈzúê?{#áwú?Tëꯕ?ZF"=Öì?|XÖ®i‰­?v¥Š¨?ïj¿/d-?xˆ'"X\?`*5é‡÷½?H»Åíü?¢ÇœŠ…m?w"0¾5?îÿ°ð€ä ?xÑ@)†Ñ?w&n	ŽL?a9›Ó=Ô?š@FrÿFµ?wSè}Ë?d­K?vg®˜4æÑ?SS"£q–g?E³—¸i!?"ΡSÆRj?u(³§[©í?ïUOGrÝ?Ç;¡u(?aá؎S?Å?iÇ=íâ?"Ü`"f?Œì*.S…?îâ3ηo?ŠÛéƒ
|?i'¢¸ñ?`ç°èe'? KÖeylÙ?ˆÞ¢|"î?íl8Naï?•,Š§­;_?ˆgpd‡)?y¶æMÕµz?±'O'8ã?"ÊC·c#ÔAGN4FGL J0828.3+4152¿ï÷fÆ|7@A˜©Þ‹;2À;›ík¨Å‡À<â{s=å>@!6ÛìOt?ýÖ`)5ƒp?ÍW³›"…¼?˜';½'v?Ιë£ýu·?úYC[öÌ¿é|O÷Æ¿îEÌþJô?Çg_	й@¿é&b@¼ß¿¬ÖI"]Í濸%^^Z(kAGNbllB3 0824+420?ìݛ»v§ì?¼›Èfbç?SXÊ¡?a+ÃŊ[?¸Å¿äÈFI?¼x‰1J-~?ï>ȖöëÉ?šW¦²|'?sUÙÕ¯W?z	¨†Ú˜?"Qª'ík?–*tXþ…?íRB¡ ‡Æ?£¶Ð@‡ ?m»« "vÉ?sºê	éÒ?´€
ž9–™?£j=KD_?ïîK;z?BmÓ5#P?P¼!céèž?EæC¿"€?œ–t€mi3?8iµô–²?é^Íù¦'O?ÈT¹¹H¿?a\´¬/¡k?mó¤ä»ªà?Ê?UFi¬þ?È!¨¤×îÇ?î†æXäóŠ?¦'	3L¶ü?x¿~zð9K?ˆf{1j)?¤yª¡4à¶?£Y0øå<W?ìÖÃñ†ë?¨V{ÛÅB}?uYÿ8y€	?yú¨á?½ó©ì‰;å?¨A·~ˆ¦j?ì†Ôozه?¢"šm‰XI?dãX­}À?b|t=ì)?»"AÀ·>?¢‰s-_ŽÐAGN4FGL J0828.6-0747?æ*ͳýs@1‡"%RDÀ:›ÇqC9À<l_˜ìËp@'ÖÃñ†ë@;™ÔQüL?ÔÖàâXz@?ä–ëip@µV=ú6'@èHÎÐÝþ?ïåÃ=×Ñä?>ê!¿ëÃÏ,ù]O¿âËñqÇÿå;Ðá.ƒ¡¿åIßG"ÔAGNbcuNVSS J082854-074854?ï…ýÙ<ÐI?ƒöfÊ÷vû?xÝ%Ì.?t•wŠ äY?'}›%Ó«¼?{¤â`ÿgˆ?íHÉ}7
]?¶4àAÕªš?§ÎWVø?²AEÕÙ-1?£¥Ös
?ž	¥ô…sS?îwQEAþ?•ìC–Ÿî?úRÍþ?†ÍWZ[ x?Ÿm˜'f'/?ÂõOÑ8<?í
ÊÐ7)Q?—ÖzžÍM5?°6g#El€?–sžö4V?m	h•‡ë?}¦ãçk®?ïŸ+s?'n³")Új?Œ¡±"WÓ`?‰q¦}±e?Œö‡Dþæ?…v?Ъœ?é6œÏH?Å»>D‰Fæ?¿ûÜç™y0?Á½@è?¶P*Š62?²´Xšj?íkS$"? Å÷Oë[?šÆüøÊ?"x¯|"V?«ëü'+N?˜€ã«°õ?çvþP}é?µ¢zêd?ǝõß?Á?µŠ÷ã?µ#ûúæ$?¼-mK‡éAGN4FGL J0828.7-2422?å4ît<h@ ÀîIõ˜À:̹-³—rÀ<\w—|@^Ù<å@
¥³Ú?Å¢7"0?šP¥<˜•@?Ö¡ô›<@f
#‹?ïÿ€³ï†5¿ç¼"¦Ò¿æ"
q¿Öž:}ªOÊ¿åïŽÎd|¿ïÿz)5ÙAGNbll3FGL J0828.8-2420NVSS J082841-241850?íÙÕû/òÈ?¡+ÆäGÁ?a‰x¨]ü?Qøìí~ö?°¥dß?Ñ? ô‹
hAf?êüè6=\`?·\•&·1­?r+ØczÕ?tóRùô6—?Ã{d²dÊ?¶é:BéV?í¦¯Ú×//?™›íÜ}?y2_VZ]L?p®G²6j–?±7[5˜®±?˜'[e@…?ïL;¼æó?lèÂ	?lL¦·v?I&wUO|e?'îö«32?j¬êB¢;¨?ê]êi?ߔ?µ!t¤)°ø?qµ"øpa?c­x
JÈÓ?Åú©Ã¢‹?´ð'Úb·…?ä	'Õß?ÆÖßd¡b?Õ¿o£?Œ6e»ÈLó?×mƒYCñ¥?Ækú¤]˜?éÄBà­ÝÒ?¨ç õ™Ï¾?ŒíÚ¨Ft?½'9ì?Ç.Õ °å?¨!'
B®‡?íížþL:…?‡Ûæ Q|q?":´ÒA²?j5P«"g?¬bçé¤B?‡)ØÖVòAGN4FGL J0829.0+1755?é¢Eàl<@=]Ù©T"À:pÓ¥¸À<t3Øt ¼@¸ÂÒ¢ú–@7·&rZ?Á=¦©¢{?¹õeó#ù"?úo|—@‡sÐÝ'¹?ïä"pB]¿Ü•)<ºEŒ¿ãðís5Â¿ÞŒ~þã ¿ê†-vZÐ0?™BüÔÒTÌAGNbllTXS 0826+180?ï'6aÍ
Æ?î'׋.?qN#Û¼©?bùŽŽ†®?†Ëò`?zæ"sôI¹?·Å[?¹FWZ3m?e»%'Fû?cê΀ù\?†£Œ÷³x?}$¤i÷)?ïGÒvØG?…Fc˜?uá6b#øä?zOZš!9?'c›ÔÞô?€q6{͍à?îäl¸ÝN?tiWµ.,²?ˆˆ™ëCÈf?cß,‰j‰K?—.óÛÂO?pRÉ£æç?îÑÈà5j?"¥ä¯?ˆBÅnÖï³?|ù™2èG?™¥O
ê?"'SŒ­?îË_ÁJ|j?›DšÂA64?yG´.1?€I>»b#? !
jòsB?–í†ìÖ?ît~K×¼6?•W	ž†µ´?ƒÖpçö?'u°|îÁ?£×¥£%$ ?'>Zú?ìÛî¿Lë?äG	KO¬? 7´§æ.?…,̬ã?±ú©%"?‹.¿÷ißAGN4FGL J0829.4+0857¿æýÖzJžà@9ÐÉûa4ÎÀ:ΖãܳËÀ<'ñŒŸ¶@6"1Rˆc@‰ek"¤?Á€¸HÜ=¿] "øáL?WP¸˜ý@PeAxEa?ïõ+Z÷[¿âH^=¢ø¾¿àÖCnÙÒ¿á`{jÚin¿ßò)é•ö¿ÕwyÿJxtAGNfsrq3FGL J0829.3+0901TXS 0826+091?ïÕ@2cï-?d'ÏÈL+õ?QéU+óÿ?Bt›óÚ?qì‡Û´¥?aú¦¯Ã°Ñ?ï–v¨9*Õ?"åY26¹?`m'{,?bPäÿˆˆ¾?†]:œÑ~?'qãtêoÃ?ïmÇɂÀd?|–Vå[6L?aҍÞÔÑô?LMKLÀÍ?µIh<?{‡K@I¶ø?ïWñrbaä?i"zÉfe6?g ¶ç,ÔZ?FÆÍB"?'ºÞµBó?h²­'Ð÷²?﹂L@?qšt¹þýk?^¿ÈRJÂÊ?QözE|.?{û¤†÷?nrŽ
æø?ï'8ܞ?"ôÚªRpÞ?f"¬X‡?k‹˜ÈÎ?™Ø"2†z?"睮]=K?îô'ƒÐ¯…?†{™2ÔY,?l¨½Iß3?aÛJc…qS?Ø—Úriä?…
 «Å`à?íýÄ*U­Ë?†6ñéÚ]?dý¬"é%?d@
¥V?¬7¦ª¦?…Á—Q÷·AGN4FGL J0829.6-1140¿íüúíÐD@/T)¥ë·À9ÍRúxׂÀ<9KWí&ß@Åq%\0?ÿÖeÒ°?µ–È®ÚôX?²†8—·?ýÄxœÉÐ@K¬Ñ¯µ?ïÿÿÊPË¿ß±$ûŒÿ¿ãì@§Ú¿Ó¯ÎD¬¿ã‰u_'®¿éÚ~Q1AGNbcu3FGL J0829.6-1137NVSS J082939-114103?ïÃlÁŸG.?wçùišv?M¡EY®K?JÏ)¸•?z•v…~•Ã?ub.W¨$?ïŠ|ÓÅ?˜X†;ßM?dó?™M}?mRVL†?ˆ#ûR‰IF?ŒŸCƌ‰?ï …›[?Õ#Q ¬?f]ç'r!f?bÁ7‡É•?œ@2g^Ȉ?\jžÈb?^›Ÿ?u|fjޔ?"E°çP ?`%Áx5fÙ? Niƒ?qÖYÁ"Ô?ïaF1ù³q?ŠAñýV†?^˜Eèá»$?T¼m;ê'V?'íµir¤&?ˆ²CÝÆo?îėÏó{k?¢pgËçÕ?y»U{ú,?‡Ó¡î Þ½? XÏ?'?ùC«Ùë¢?îU'¥?œ¾â…DÊ?ws»³ÿ²6?rf¼wíì?¬Ü8eý(î?›­ °G?ìŽä}[\?'è›d"á?š~7~Í?}e8C‰[Ð?µ˜#=jñ?ŽR³?Ø¿AGN4FGL J0829.7+5105¿ÐÏgÖAÚZ@Aûd­ÿ',À;A³àl½À<ÛãÛÝ@˜¥ûý'ç?ÿµA*l»?ÎK`æõ—ò?¬øƒcø"?á!aRüQ?ûZÈΪ¿æv!ÅL¥Ë¿à…'âr%Œ¿ä¡‡¿}¿ªcÃ|t£¿ïÿ"Àh¡?ïóÕðaýKAGNbllGB6 J0829+5108?︪h@S?u #åxl?a›Óè@aí?ZKøžY>W?{%ÀÐàmÂ?rÒõS©HW?ïpX3·P?'£–à'+µ?lÆ?yÆu/?{ït=ÓÃâ?Œ¸c?\º«?‰NÁÑhŠO?î±wT?•†kG)h?'*±mh?"¡èêÜú? JÍâ)3?'e1`‰Ó_?ï|‰½Gb"?pôUÛàX?p«kvA?ZÔm¥"½?ˆÕÕYýç?kՕÔ)@Î?ïud§ä#ð?ˆ÷6ð¼r?qøZÚkÒ?p%,±Ð!_?‰ª¨Ê›—?"e†¦ù?î¼	Šõ?¡V‹ü)t?y¾íÿ?ƒò⨱°?¡÷òß=å?Oÿð?퐫¾§Ø?Ÿå'*ŸŒ?ˆé®1ý!?‡ÖP—ō?°]l8T³ ?ïW®g²?îh®<"Ú?ør¬•«Á?…0ÞwÈ
?v½D½øà-?¤(ä³oï×?ŒƒìWÿAGN4FGL J0829.7-5856¿áÜ·jSËÀ'÷¾æÀ9Œòã·ÊÝÀ<<ʋ©í@J€×¬@€Á@§ü?µØáò½'?³HÐ(ví?ûˆ5©/8Ó@éI&÷ç¿ÔI":<'¿å§zޢ߿çÖj¥Gá¿æ¯qr3#C¿ð?ïÆ1bM§ÿAGNbcu3FGL J0830.3-5855PMN J0829-5856?îUI´&:?±Ø˜¥+\Ë? Ÿí™«Ë?°¤½Ž;M¦?"î;Ùá8?˜Å^èotë?ï
ûåÖ©?¤§‰.Wû@?zò'pŸÂ?†kmý­—?—ãß­Cù?¡=prà›?îu]½JxÊ?•Ö ã7?vÜÚו?Œ´ Ï"]? Ìòiï|?JU'¡, ?ï3Uj?¹Ô?wþ~Ú«N¤?~ruíLñ?bù]œ6Û ?'øµS¡w:?sginË?îTwP:ø?ªÑȺ7'?Œ.æBJÅz?œD33ÿ£ô?£´úiŸ?¤W$G'î?í(œ—XQ?¼¢@Wð2?"d‹RàÌ?¦¹µgKB?±á÷ãC4G?¹GGñ&
?ìuÛÿ¤?¦ßJ€Oó?¢™]{߉?—Ñ\ièoù?³S¬zí™? ¡^?='?íOêµ	?œ•P¡½†\?›øxf	Î?‹Š­R¼?­	å*=u"?"Brµ°ûAGN4FGL J0830.0+5231¿ìœ·…+½7@Aÿz¢]zÀ;ðG%XÀ<¼•¹:I@ žBFK"?ÿƺ~ìo*?Ι>ív?~r‡î¿?ªDOÿáeû@ÍãùI¿å -à
¿ÜÜ
œö›R?îÞ!¯é¿ßu¸ÿ:ˆ<¿ìwÛ~kjÝ?ÛF.b"óèAGNbcuRX J0830.1+5230?ïmŒi?Šdð'ðO?bÞ^^eü?Y.¹˜fåz?±
Ê0?ˆþJÆ?ï¼v¯E
·?€4•U·?V/Éõ–•d?c,B
V
?|8µô±&Û?y:ÔÌOkO?î»b"ãÔ?': -	2
?{q«^»ì?|תnvÖ? Û¶EÛË?Mí¨µš?ï‹GJ'§ ?oOÁރ?ZHÂ:œcñ?N‡£š"¯ ?‰å8¹iu?l}ßù€,1?î†äDQ'm?£ƒ¶ÔÀ/?s(‹Zý˜?jG»x?¥,ªG°¦x?¢¹wãïÜ¥?ïH@#í¬'?˜;‹s'?dS0ÅÂÜÒ?s.ëʨØ?"m•g'[•?–
qßi¨'?í°aŒŒë¶?m÷æg8Ú?ÿaèýu?€ÑËQ´?°=_TÞ?›
Æä–È"?îÊwµ¹(?ŒýÚ£ßt˜?gœ¸ÀJèB?g6;9µ­õ?¡Þ¹!]î?‹íàþ§AGN4FGL J0830.1-0946?ص™Öf½@0ÊFà!qÀ;A8"ÀõÀ<©!6±m@ ìcÎ[˜,?ý°áxÚ?Ìh´‰ßè3?£ý?[_¢'?Ü:…M\T@?%ƒr:Û?ïÿùSt¿èýÒ~<›è¿ßŠ'¥aMù¿â9gàd`¿©¶I¨•Šì¿àÚ¡'µ AGNbcu1RXS J083014.6-094455?ïð³Ü»Ø?'@7ûrÊ?4¶JìRTÄ?1_³·ï?‡Þ ŸAU3?'!¡s)XÄ?ïN¡–Æ´
?¡Úa´¼?b2Ä]E‹?p²á*4?"åt•Q?›ç›a>}?í×fêMnÑ?£²Mz?WàSÎ(?bŽîºÇ2w?°åGacST?£±³R
¥?ïµu€`/?d—nýË?4lÜk÷+?"\<‹ ?ÿ9+ÓÂ?cæ:"Íî:?îș^,Ój?¡¼ž¨ó?GÝÏ?ú?CÏ:á<p?£ùÄZ@?¡™êÜ´Ì?î«äy*¨?­'ªâ
É?d÷ªC§sô?uCÏ9€ï?£ò=Í$'Z?¬æýž¨|?ìXhÅfQ?«	2r‡Ë«?[OLßxÁH?bþV{š|¯?¼ÒŸ…Òùs?ªõôó=?î÷K›´ÑÙ?"ó•yÔvG?K‹7ù?C0é1ªe? ÏëÀL?…
õ•Ï‡AGN4FGL J0830.8+2410?à_>±ºo@?ÛøvžÂÎÀ8´wcä¬À;܋Hþƒ@ÿ).L™Œ@L±:?¦SN† Ã"?À³Eý9@ù/+f¶@—Šh"¿×ÔÁû¿ã9[e¿æà›$´¿é:귙^á¿ì½Ú@¨¼¢¿ïÿïXzAGNFSRQ3FGL J0830.7+2408S3 0827+24?ïÁz.wë'?x`f#uÒ÷?rí"ø$"?p°t£J?hª©qˆð]?e]ˆ""æ?ïؤ¡µqç?wÀš•ê é?F<"T½ª?S²»oÕjs?p暎×?v~Œ:	?ïnKdØFÓ?‹Ø­úI?wbHúß?€zÑB(t¸?ˆ¼&¦ ÕQ?"¥…äo¦?ïûõï'b?&~ÐB¤	
?Õ,^ÒDe?‹älã_?8›=¡'¼?#+ã x@S?ïb¨ü¸ø¯?šŽOFF?'¢š¯â¡?‰èÏÎ4Y?"³&ÂéGw?Ëö¾+×ò?Þò>K?†Ž 
Ydz?ZNkCØv?iw¥ay›»?…U:åœ6?"rà¡m?ï%PHº%x?"xL¶Ê©r?uC;ÏÂt?É2 '*?–(#ƒ¿r?'òEø'?ïõ‹ØeÝ*?Dçñݯ{<?5w;èÓ%?*9å/¹‰ ?O%U³?AÕië®PAGN4FGL J0831.4+2631¿ì-'Åjü@@ZŒÞ 3èÀ:یwr'eÀ<r7€ŸÍ@í5eèg2@+Iº?Ê°9FÅ?¢ô¤­Ï?Öin¼ó¼@ëpõ3s¿ãà]¾!8_¿áË¿¹Ó¿ê'Úgê¿ÞØ|ßy£¿ïýĆ­-Ë¿îÍ´Þïd&AGNbcu3FGL J0830.8+2629MG2 J083121+2629?ï½g_P6?uhý"Ðz?]ËSr½:Ÿ?R‡2ÑÈæâ?yٜŒeÆ?rÚjêæ†?ïÃ
!aà¬?x=IÃâ¨4?T•I#ǜÃ?^«m¢‰ô?yTl–Ð?rכZ(ˆg?ïhÍËi9C?y1ƶÈ?kÅ~ž¾?`¦ÑLО'?ŽÛ-¤G;?u­ùV§Y[?ï‰mÄv'?g·¦¾#öW?l|.`Mæ?OñGªÓ?†…ƒ:œ.?d6G`ûç?ï|ùõÇ9\?…)RË=?m™Ñ-GÌs?cª]A¿³?‰[H·Â?'rP"›¾?ïGËõós?"5`W)?eœ]ë®êX?r˜6¹¯Ì?"iúÃË´X?'#1b—‡˜?î»°N€°X?Ž2
H†å4?z"Ð{4T?rä~(?¡¡	¬Ot?ŠdSSɇœ?=jĚ?†ÑgÏ¼(?'âbÊËKá?npǁ#?ŸÝ&冧Û?ƒÙz.î¶AGN4FGL J0831.5+1747?îÿÈï·L@=Úþ£ßm¹À:µq5ÍÀ<~ùÛ"Ðå@ ¤ßðbÿ?ü2ÑɋϬ?È	¤"ZS?ÈBY@ãö@¡³CŽË	@?Ücï(
u¤ÇË?ïãՂS?ǒ£Ì´ú¿ÝiÀ8î¿Ýïø€¯½È¿æ«œ 1£¼AGNbllGB6 J0831+1746?ïÆ`‡²Äì?,èáîV'?Tƒ¡R}?fJ'3©E?wž å!/?‡ÐÈ "þ?ï׎‰ñ?r'Ú-î-Ð?M'Y^ß?UçôhýM?p†oã={?kêpÈÔ="?/>BA?€Wå&XVö?]®ýð?cHý&1D'?ŠT{m¹¶?"'Åß.?ïSwè*1"?nw°}þL?p¬%zrhÑ?SÆÞs'Í?'eù"†-w?jÛ3½(?ï³/Ίù)?z2ÂÒÒ?^7ßÁüL2?Y0©ƒƒ?~Ú ¿µ"~?u¾ÌËÌyò?ïŒèjÚ`Ö?ˆ8Yˆ"?\ºdžœÚ?eäˆ'Hâ?‰.˜©5—1?…3…'Å|Ü?ï9]~á1‰?…wƒö?eûv·ü	?jõ¤éK6?–áNêå?ƒ6A•T›?îŠÞaòA?†Pë|{¬?|ƒÿä‡?®?j_ŸäÀ–)?£ÁŸ°Õu?"SêOùïCAGN4FGL J0831.8+0429?æzf©_èÑ@8YVŸIÀ8,vü¶ŸdÀ;«UãTÏ@yïJ%=&@rN¨Ú?-ÞM?³{1yŸ©(@ÃÉîËû@;ț9×½¿È••~Å¿ß4ä"ÔÁ8¿å$ŽTÁù¿ãŸLa¢—¿èþ5$¤û¿éáä¡ÂAGNbll3FGL J0831.9+0430PKS 0829+046?ïîÌu}ÊJ?Pþ±ê|ð?@MòfY‡?0;‹ÿþ¾?Zdî\¨g?MlÇ53j?ïÇhõÀi›?z1AË
W­?P­–ãq(?YXGNO´?x qí¨™?wH5ÄÍì?ﺜDTÿÈ? ãöA2Î?Xâüëê?aº˜dá¼(?|yUÂWe†?|ÎT¯¦?ïðͼ¥§??;	͝Á?>ìCÿlô?&âq#?V©ux]Ïá?9"'Yp&ý?ïÜP'_À?c#ic‰MÚ?=K®ØîDY?0yTÐíi?p	!§?bwñ6b4w?ïg¥7÷,?˜`ëWÕ¿?dV0f¹Ã<?tÎÊ	H?'åTÀè?–"R
Dï¢?ïª8#÷šÆ?™`dé?`lJᏤf?jåˆÊÝ;?VäT´%w?~m­ê ÓŽ?ïßïƒm?[ڗ'
µ?PŠáŀEì?C^A9õ?h›Ÿæâ8?VyÆÃÝà§AGN4FGL J0832.2+2753?ÚÆp8"…@@ ì•¿ðEÀ;8^B«v;À<¨PŸTÄ}@"Ô¿Šo@'™Ù;?П‹€Ò"w?¿_ë^C"d?ìv¥CÃ?ø3 Ä̊?ïñ`®–¿äë‰>ÿàK08¬ð¿å՟¿MˆI¿êg+R"!‹¿¶‡ä‰ŠÙAGNbcuOJ 250?ï'֙1ó?'"í$Œû?gíÕBS—ñ?bœþP¡-?˜*†Ÿ–?ˆt¼Æ?îø"öqƒG?˜"q/¥Ü‰?ƒy19?''8>?—z nż?"a;é?îñk´üBþ?ŒÝ>ËG¯?Fw5ÔÑ?Žˆ§–v?šë™]âô?‡^ájqA?î-}çŒk´?€±Œ'•?uOFëõþ?oùȦ?¤íyå{Ä?zŠÏPÛ?íÆQý	Ü?¤…*ùWÚ?'ËUô"?$?y¸½\%Ÿ"?®è
³Ëö?£rC¹-?íavaŽ?®-
«ˆ?–MÂP~ý?ž°®/¿"?®Á¸ÅÏo¤?¥v"¥ByŠ?íéËà‹?™¥#îû(ˆ?Š3)K½?ƒ›VG^›?ªÞõ-$?•ø‡N%m?êò>=tÌþ?œàqLß?¡!Ï°N^?×3ˆ7?¿Ý,pá?™'®¤ cÖAGN4FGL J0832.4+4912?ì݉èe@B1yЦv!À:A0«™v^À<˜Ç¤nß²@¾]r¡Þ@¾\ǁ3?µõÞ;¿ŠS‡;žÍ?ԘÂÚô?÷÷/™Ë˜š¿ßÞ¿þÞ÷¿ãc-ÌÁå¿æ®x?'æ¿ãU1Š¼‡¿å%yœÝò¿äF="†AGNbll3FGL J0832.6+4914OJ 448?ï§âh{¥¤?}h®]בÄ?T‰gP¨ÛG?Hö÷tÉ8÷?ƒv8þŸŽ?|jÛm¹?ØÊ~`?‡ ¥Ì^¼?lœ}%yôÿ?tyêÒDNš?‡°ªwûH½?~¸UݲA>?ï
ó´±è?Šî-$š?""¢«áÒ?…¹œ=?"^P/|Ì-?'=iqÐ~:?ï?•ãñEl?tOgÞ>ñÏ?‰býXäPU?lT,Ø?†·‰µ(¥?e±‹U"ÿ?ïº0Ï?'û»	ÇM3?iG¾©ø"B?^Pvuâ4?šÿÂ'ð?'pŽ`ê÷;?î~ný'¢J?£"ÓTtx,?ƒÿ…Ëá‰?ÃyZíˆð?£N¤ï{?žÈ¿´ÑÒr?î[OhëHZ?•|
E0ê6?'9
ãˆÐô?
K×pŸ?¡®"ÆÝ?‹z™Cö?íåLüÄ‹?'bm"uEç?¢["Â[L?‹]<KSÉ'?žŸVå…þ?'ý—¹ÓG|AGN4FGL J0833.4-0458¿ìÏÉVu®@4+"Ù@yÀ;çÌ,"ÝÀ<èj±NÂ@¦9$¹È¹?ú6çÚ+?Ôö+ÀÎð?åÞN4@ym@››]@'~ã	û?ﮔ"6`º?ְߛÜiù? +€À"À¿àvH¿ïÿ­?å`¿È~£®$kAGNfsrqPMN J0833-0454?á?A±º?Æ ÿe6¡¹?Û<Úý?ÆJgSžf?£…{³\s?›6^ÒAƒ?äî¦g÷ú½?ˍBü²?ÏÙAÁ&·‹?ǹ¬42?¸ØI;Ìù‡?°s«u9=?ߓOҀŠ?µl7ßàé?ُÅ$·ÅT?´û(v¦?»s¬[Nk"?£Ü@FçÑþ?ëR5EËÕñ?šË9ÈÐH??µß[Ïƒ?˜_OÛZeC?¯ô"76í?‰z֌žq?Þ±JIic?äÄBî×?Ük£ï€M?Ä\Yx¨n…?³Ž¨J/¥¿?ª2†X&æ&?à#ï 3Ò?ÍYtñ±}?֓åxràü?ÌW¨")V!?ÂHxŒ%49?¸–­ꅪ?Óÿv¼¹ž?´áÈèì±ý?áìdLj?·áÀP¼?ÀO'-[É?¨NéW~r?ç<×pXœh?¬³¸ÀۏÏ?¿þå«èÀ?©§Í1ÄX?Ã
/·í[|?£QºÏ¨ðMIXED4FGL J0833.9+4223¿ì»2Ôú©æ@B"ÂÎFIÀ9Û‡\€4À<uJïèZÈ@#S—+Ö@<A<
rJ?³ìhžyþ?¥z{TDP?ðœí¬@eK@
U€ºûi?ïþ,‹yEf¿âϕ¿ol¿ç'K³žÓ¿àmš7NJç¿í§VPn­]¿ïñÍ!ÜHÁAGNfsrq3FGL J0834.1+4223OJ 451?ïßYÓAA?b3²í¥å?LTàkÇ:?Pwªê³L?iênôõ^?^—ösê©q?ï¦{¸Ä=m?¦»?WY?gÙÄF1bÝ?~L¢&/?€j ËÒ§Þ?iÁE!Ä?ïšHr¬è"?ƒÜÅ®m?sÏÁ=áX¾?€,Tä2@?}ˆù?qâ¸G2Ý6?ï—0ËF\R?j¢Ý«è^Í?}K‡–K?b¶M@dóï?wJNÕ;‹e?Z)>ãÁ?ï±E
²FË?w·ž©¯)Ž?`ôÂ@¡Á?YýÃg+ÞÚ?~ã¨8<?v
ôD=ý&?ï=f4è??›ž
3Ô ?r	e$4!L?‡vÐR#Ÿ?"Ðà ÊL€?"‡Åû…š?ïUÀE¢C?ˆžåá:?}lá¦âÑ?'p^Èý¨?‹Ù}Ô$§?}Ô96Ý(¼?îÊ0æ°VR?Šøj&½¡?—Ç]?"d´ºNFg?J¦¾Üy\?w£
lFAGN4FGL J0834.6+4402?é\?j'ß°@BFK†ýÀ:yÞfRDÀ<§—L¸?w@Ý(bŸ²b@CF uÁM?¿iS֖Ð?½§Žú¯34?üK‡mG+8@	E…a~J3?ﭓK¡¿¿s?|0–åy¿äO›HÆBo¿ãð`̞¿á²¬ÅÆHN¿ïü:]Éß³AGNbll3FGL J0834.7+4403B3 0831+442?ïí'vD3?Tné×D?<®©Ÿâ¦?.ap'XÆ?]šތÙë?R€²E͈?ïØ°"Ý?r4'&`kj?I§hë'êÖ?S[ªí÷6O?ps‹/À?mpѤLü?ﺑäE?oîÿ®™'?X˜3°7"?`‡(8
yš?|'{ÏÄwã?j¡'Šù?ﷂ¹¿e?Z$Vð~b?nKøÈôf?N( €ëäþ?u¦ÆÒ­?S	5ûýv?ïÙžzBÖ?eÍÜ/Øî?PyéG?DÝíj?nÂm(ô<?c?™xÕ?ïŒ@Õ›8?‡N=®>õ½?[§<–õ'?eÚ2Üæ;?‰zãòP?"(ºñu?×Wóº?vvÿ¤f'?a]6)U«?aÏ¡Åå`m?†¼š–ü?rÝ×h\ŒÕ?ï@Ø5>Xß?v|«J鬰?'Ñÿ{œ?j*-Ô?Œ÷óDš^?pr÷jAAGN4FGL J0835.0+6243¿ìÁŘâ @AÙGNΚÀ:ê"@lÚÀ<ˆ$GÝå#@SÒ¾SbS@<=3g6?øŠØ¡e?¬À'¤)añ?Ø9ºáè¾?úu…•Ö–z?ïþÛ½«q³¿èÝ¡ÜF¿ífÒ1›Ä¿êŸ—£ö¿ïJ˜ñÓí¿ÞÃÓߐžÉAGNbcuGB6 J0834+6249?îÇZ¹xËÝ?¸è ÃÍ}T?•(4úÒ|?¸*|yççI?'ì'¤'·È?›j6—¦+L?îíçY¸%?¬!)XY}?ˆÃÇFyVÆ?Ÿª'Ø´wñ?•á;N´?¤n°:Y"?ì"N
?¥í!儳ì?žªC
…t€?šÊ=,Yšé?·Ü[2œ-Ÿ?¢gŒ.¶?ï ÒïŒÑp?€e§¯ñ$?`÷ª·SS?mÉ`ÎÐFÐ?ƒYz³»?xÑ-›úàò?ïu?©Ý×b®Ê?†uO"-?¨£¬ãm?"öÖFÚ@9?"ÛYb^õ?ì"vä°:½?Éf#Sê?¦ ">Äw?»mR'˜q?°Kþ½•	X?µ¶ŽVäK?ë瞏¢ŸÓ?¥>ÁÕ0?¡¤hÐZI?›&È·V}l?·ð×âH? œà¿Ö–»?î/•jS?³Pq=È?múB<ï¬A?'d[-Ôø¶?¥b$&Œ?²4§áâ±ÜAGN4FGL J0835.2-2243?íå_â¤â@%›™N?À;>ŒjÜí¬À<߄ۜsi@@'I}"@	ۛœ©?Ö £ylS?ïÿülò@ÿ3å	Út?ÿ4]q +?ïñô¿Zƒ¿á½Zi¿àøú'0?¿íÔ-ê¿ïîÌț¿ííËJÍÈAGNfsrqPMN J0834-2241	?ßÆrQùiZ?Ì 99¢?ÖÁG-;!"?̘WÝ8?Âð¼« ?¹ÇñÂ`ÉU?Ð)7G{$ö?Ìla)]ø?áÂΜ/Ì?̨OxQ?Ëz†6˜öå?ŸªxÁ?âK.çôñY?´ØF±öŽ?ɟõÅ$Èó?­G¶Èµƒ3?Í3N-3%?¯{^Øîè?Ó·îÿQ¯J?®›NËK4µ?ä"Q[CH?°œèdC?°
»¾'Zœ?™O]¶>–?Øx¥Ñ"ä?ÉÓæ
zF1?ÛÂÁeæcÍ?ÌɋÓ÷þ?lj1'od?¿»áƒ?Á<y`œ«z?ÄÃ2ò=-?äV¾y²?ÏL¹2!vƒ?Íi©/<?Ç8ƒÃÞ+?Ûy{tž2?µIØúÎ)ÿ?ÑüPI)ÐÅ?³`Ûcj=?Ҋ4CJúÇ?²ñv²½?¶€^ãçÐÇ? šxê1›?êd33'°u?°:?|M˓?¶^~®Ä•?§#:ê5MIXED4FGL J0835.7+0936¿é T5ƒ¼Û@;"È6eÛÀ:ÛÉÃ-ÚÀ<Š€Þ·°Ü@Êõ7O!¦@·{¿"ÿ&?ȂÛgj?¦"¶]Ÿ˜?ã—ñ=Å]m@ ÄÃéÏ<?ïûB0&8¿Á%l5³@4¿ç¾"7Z	¿ß@\[˂˿ål¯UÀô¿àÍÛÀ…—AGNbll3FGL J0835.4+0930GB6 J0835+0936?ïÉåIÎÞ¨?f4ñ·¶=?J¤N±e¡¾?<"]Æ÷"?w¸Ñ5óÈ?dÝ*;‡?ïÎпíã•?pR•]N¬?K$%5ºÅî?Qi>°.ym?u3bhtB?jæRY'<?ï›ódw_?vdË7" ?[ f3Ìå?Q;f°?…ÈöX«J™?u±êé+t?ï™þîµ?`Èv‡‹ò?dGnÝc?B$n'ŽqJ?"©dÒbný?_³Aʞt?ï§;}Qù?y#وxÞ?T…®wA•û?F§­"¯?ƒ jÍ`þ?wwI¡(k?ïˆ9"/ã?…9ºÆ@êÌ?W}ba` ‰?a†¾å4?‹î§Y?ƒµÚâv?ïR²8>Ÿ?€	N¦ŠÒ"?e‹/²këÀ?a´ªD¡?Œ?'øS¶Y¨?}á‹)íü?îÄÎÝâã~?}}ÅOðK4?}ü ˆê ?b0fÏÁ?ŸæüÔC'?zùóé83AGN4FGL J0836.2+2141¿âåà1X'"@@'óUÎÀ:+?› 'À<b¶FxŠU@ìõ[â(ÿ@ö+ —ºœ?¹|ZÞr習"¼\‰/?Ôg˜*-Ðô@	õ½©Ä4"?¿É읢'½¿æ©ÛÑLŽN¿ébÇ«$ÜX¿å<÷‡¿ïtRQÜl¿íoÙ¬¯ AGNbcu3FGL J0836.3+2143MG2 J083615+2138?ïð̍Ú,?m€(ðÚÅ?@"[à?8uUƒXï?V$Û꿁?lÖÞSöâÌ?ïÔ­†¶h?u8A©nK?MK_ñÍxF?WÅž7J³?qÿЍ%1Þ?pŠj"Mûc?ïÀs0+õZ?h»óRFð'?Wù"î?EQS6+¾?yÈ#µÞ¾þ?g°ÿ—õ]?ïÒÿ³ÌB0?T6ª
#ö"?b'Áˆšq?Gœ§RkQ?j}ŠƒGæÓ?Jn‡ã‰X?ïçKdh›†?`Ôâ3&?NŒ¤Ø2¬?B"Jã"Üæ?arrºY?\Ã+¦[zÎ?ïˆÚŽEAl?Œ#ª÷\dÒ?`»!ZC?pÜԃܸ7?‰šxm£<H?…ðÎӚîÅ?4?ø"?{Fd‹ki?aêl{A}?]IŸ÷ý¶"?‰YÝè	1?xùµ@o­÷?ïs¯•?wÈGÂ5hó?€*÷'*µ?n¬5>7A?'÷'–?jyãâŽ8;AGN4FGL J0836.5-2026?ËyÖ꡸¼@(9	(­ûÀ9ÞØ-SbÀ<&æ"Gp@rxJ"xÈ@¢|—*T?Ã([!?Ò7ö{ò¿¦@)È»ÆL@	ÒÀº컿ÝÑK·Žw¿ãŒk'fL¿ìæMÂ*²[¿ïÞï@4£¿ð?ïÿþBe«+AGNfsrq3FGL J0836.5-2020PKS 0834-20?﷚=$ðó?'küÑG4?f/zˆÞ"¥?lBñ¢0JW?y$jÑ?}D_Ôôˆ?î•SÂÛîd?®áîøÓ?Š1oH>0ˆ?˜]/5@·R? gûæ
¤?¨WOºUæa?íbֆVh?¢Ô_Ëê-?¡ÛJWÖÅc?šÓ!¢'?¬>ˆ<T8?› s	˜?屢ìCî?l>	2?pˆåQàë»?ZÂïÂä?|±$wD	c?c¶&
âL]?ïžNP´½%?Œl7Yà?sZ st49?€Ô¶'©æ?}~7)î))?ƒ6|›ƒ3?ì B;±»?ÃóŸ¨ë‹?©<bPÂ&?¸«ü6‹œ?²_¾ŽÕø?·ßÏ"±h•?ì|߄èæ?¥™%î`¢+?¥C	?ï?™îZ°–¹?±w:ä%±?Ÿ—¢Ân?îÜ"øtè­?öÆÉ?Š¥«€êX?}|¯¡Ã\ª?—(Ë,7G?ƒzß®Ç'AGN4FGL J0836.9+5833?à_Ú8α@BDaAcwŸÀ:ÆWꢠ©À<¦­@?‹0@¡¸Ðìl$@º:Þù;?¸a.n'z³íPÑ?ñ–¿Ê…Ë?ýq
×tp•¿ÜÏ|¿ïÒ¿áN
>¬ãù¿çh?ŸR@?¿âj4¼ .ß¿ã"2þ¿Ø­JÜKAGNbllNVSS J083705+583151?ïÌL©ü¾,?fɌ¸ùóÚ?TÊj¿¼£?BÏSÈ
?t§˜Þ¤?d{Ìl'6?ï…ð[Œ£?…AÖ!$áã?hv,8äi?q5ÀB|?ˆ}K'@24?OÖ	¿úà?ï_:Ùg1?€#"Ÿ~ÉÖ?p¦ºÂpÁÌ?s‡m°Ø?ê"ãöTÉ?w™¶"¿Íu?ïFÃQq?p}Gl8×õ?~(¶}×þ?\óù4}k×?Lνµ?nmÖôW?ï'70
?{cݲé¹?gë ³Ëg?U"vª7?…°y!W}:?xyûFŨ?îºrªlz¨?›}Ãߚ-3?xÀA³&'?ƒ,ƒ$ÿ?¡@Í%'Tº?–ä˜9úø?îáRƒŽ?‰RÌüú?{P"ÿÃ?y§?š­¿c?œûÑ譍s?"dõ†Øt?í'Õn÷Ú?ðåKlç"?™¹­‰œ"?ƒ?"§V?ªö,_·ÿ?‹ÒV–¾±AGN4FGL J0837.3+1458¿ï"Y¥¢@>ȼœÓáÀ;)(Fp&ÚÀ<§p¶K@ ö
³\Z?ú'¢ê{3}?ÖÒ"4ÕË?Áéoo¦V?ñ¢.x¹OB?ý1D‹u>›¿ï±E½yr³?ï;ˆÂ0ç~¿éT•]õ©?5n&NHbo¿ÞëF'¿àª|uœdOAGNbllRGB J0837+149?ïÉcäßpÇ?jE}ZÅ-§?D¹pâú"Ä?<À¶ۜÏ?x¶ß‰Â¨Þ?hwÏù?ïÁ½ÚÁ'?xd4רì?R±[jÔq?X"%
]?zt»¦MHë?tœ3õo?ïWcë{¨?€v‹|¿Q?g{<¸ KŒ?j4¶4iÇú?'/‹óc›x?|P²2_SC?îëyï–a'?|²uÏmr?q¤5è»Þò?Z;)´ŸÓq?ž'´—$]þ?zãFíÂi0?ï§c®r'?uy"Xó>Ú?U	%íG?N?ŒƒÄÑ?ƒ…ï¡@µ…?sÞÜļˆ?ï[³@Îk!?þ«ÔB?dP•7~?qP{êóXœ?'õíÏÉ"ì?‹ÔÄ©A÷)?î¼xðñ^?ÝTð¢]ñ?pËÏm,P…?q}Ioö3)?¢÷6y?%O‹Q®ÿ?í]À–nÓ?—4ü~C¼h?|{;(UÏ·?rÆ7ð!ߥ?³JGšo?–†3ª4CAGN4FGL J0839.4+1803?îõZ»ê@?¶·ª%ÙÀ:`þU/ÝÀ<€VAU5@ùZ<a…@Ž±=û
R?¶Ðó-‰¦¿œ܃yË?å±
õ´M@»<.Y"¬¿ËßÀ‹t¿ÞZ~¦¤¿ä	`0Â?«¿åJŸb0w¿á•`Nõ1¿ÌBEÈa-AGNbll3FGL J0839.6+1803TXS 0836+182?ïèÂÄúà?XVFDå?CcZ/Ò?BÿÜ©u?b—f­ÃÑ?STUÓ(T?ïä!`´?iÏYüîü?;5×´ìþ?GCé—Ç—?hwä{Ò$?eÜ´W}Bà?ï«
ÝÊ·?tw9H|?É?W×!éšû?U¡6ݓï¹?'A¤vªžÕ?s3gQÛ?ïÓXß?PÔ{€ËŠ·?Q¥¢"up?2§
˜+å5?qê(¹
v?OÕiøºÆ?ïÏ?1)~æ?e{ÿQo¹j?S óȤ?B¢×¨
ªZ?s˜cQq¬R?czB"þŸe?ﱄ®"Â3?Ó¦ÚA£è?N˱-P
¶?[œ,ûþÂ?²Bö7"?¦¹Û24?ïeTåNg±?€ÃÖÙ<(?c(mÑüvÝ?\qL­D'?ðU"?-Ø´™E¨?ïz̀sOO?p"7ž'v?hérR¡?T…ÝöUZ?‹C\G¿â?okÎøþ†gAGN4FGL J0839.7+3540?ÄKÛÃ>f@BA,üœÀ:RÆvqvÀ<ozLÍ8-@ãÿ:³/B?þ¬€&+
?ºÛâ~å¹-?¶$[T ?ü§‡H^=£@çV:õ?ïþ7+æ8¿â¨Oªb>¹¿ÙÀ[¥B¿ÝP»>Z¿álšÈmÂ{¿â	P
ÚN–AGNbll3FGL J0839.6+3538NVSS J083943+354001?ïÐóM/ã?e•Ÿ±?O4QÑ.X?[W´‹O6o?sŸÏic^³?^z?)í)†?ﰝŽ¼¶?z~;Cõ¶?[b
ø2L?aoñB¸V?€lw©(=?tGšmÞæ?ïse½ÉúŠ?vǨڮÿ‰?gJéË?czqÄí?TÝø'Ù?rûdÒoç?îéq}ñg?pRPPÁ?ƒÿë«ßÀ8?Z½\	rÇ×?˜ÑÚlŒ_
?kÇ©{Ô¬©?fl–Œ±?o>…R	*?_N÷pϟà?`Éô9% -?€õ{{y- ?j¾ÓñÌd?ï/*%sÇ?'y€Ùáµ?o½ ÁJrs?vM͸b(?–#%ò×?Œcܘ}"?î♞ˆR?Š¨×1ý—?u_~ž¡*Z?r"'É}?žT숭LÐ?‡Î)ë|^?íHB?‰6µ»ç‹æ?–&mÞòí‡?tfÀû¨©?°5"äz¾?†³÷ehAGN4FGL J0839.8+0105?ÙphJ
·›@8uà'Œ6ÛÀ9™'ÿùJÀ<Êþì@æAzɟÇ@î][$éÄ?µŽOŸ¶¥T?ȟ©érõÁ@ÂÇut÷#@~‹ž":¿ÓÐÂÛ\\¢¿à"0±x³p¿äSø:8àò¿æýNª‡þg¿ïþôx
¿ášXÜ:(AGNfsrq3FGL J0839.5+0102PKS 0837+012?ï–åÈyßs?}Vá݃êã?ÌÇcÂJO?wÐÃQxî~?póX¥ì?dŽA¼'æ›?ï¼ëµ½‰?|õüè9·÷?^ƒË¸5ø?f\çl¼´?yé2Àãæ?u«-¬gÒÏ?î̝ùœ†?—NMY¾Ñü?–Ì 9îN­?"ˆ(•æÕ¹???ýÑ:?‡²$Q"\:?ï½J•>Yò?ZþD.O>?ef"õÐ-(?G³1:7W?v§kV¼®?Sæ^ÆðKû?ï1«¦·d[?`=¹fA?'‹ˆúä?Š"sçb¸"?€	:³OŽ?wéõÊðp??ïAeìK Æ?–¦èƒä0?tA:D5ð@?ƒÂåÐüG¿?'Âóç
>1?RΉ.u0?íy ø³…~?£§ì¾?§¼™á®\?žˆJä@6? ©V–ˆÄ¿?"'QG~p?ïO'Uò>»?x´a¢Ê¬?{PÂak?dº™"÷('?Žs_¡Ø?rΪѲ<AGN4FGL J0840.8+1317?ç¾:"¥¡@>10ߛÜjÀ:"ÒÊ<ϔÀ<s¿T>E¶@¼è7"î@ᶃµ+Æ?ǜvXKñp?е£»[‹A@9E'Á@ÚEÚ)ו?Å?ïÚê¿áGïþU0¿èŒoz^Ù¿ä0|ŸÏ¿ð¿ïù^Æ^ô'AGNssrq3FGL J0840.8+13153C 207?ïٜµÇ'h?jà"‡c?^kÝ!š`¿?XÌíS2?g-['£ç]?c®Æ˜¨r?ïÚ4JE¯ž?q%Cõ'?JKWW#!k?U¿<B/ã?o8ß¡?j€ùóH"?ïU¼öý:?‹Ýø­Ì¦?€š2·ˆ{
?"þ #Xl?‰ö'$r`?€Ä! Q[?ïÐ[¼X$H?Rɾct6è?^çd·¿f^??þ#"¬5X?pHP–w?Mé³x±f¶?ï°m¯'m?zY£Îf€ï?qEè"?o;°¥Ê ?v܃Khüö?q—ü¼?ïŒ@ZŽ?ˆÜГm¯?`½H‡šžë?kOš+–°?ˆÀ—>³_?…FG<H"i?îÅ6ܗ?"ÈpCJ\¹?ˆ4â8X†á?…šeòM9ð?›>ÌFÿ"«?Žo(–qýæ?ïu¸¢Y—Ý?rgHìƒô?u‡rNøÈÁ?\ÈJN[A?‡ÎRóºD?nÁäDÅMCAGN4FGL J0841.3-3554?çˆè>ö¾k@
î¦]¨À9ÃOu‰À;š$ˑc@ X¢õãÇe?øáS½vd?´kë
¥u?Ê:
Âá@d¼~ ïÏ@áé{Vw¿îHPÑ©«?ș5[+ŸÁ¿Ì}†éh¹Ó¿ÆÀUÛ~ÁQ¿Þâ›ìK¿çÏ,ù]OAGNbll3FGL J0841.3-3554NVSS J084121-355506?ï™L«Õ?§]N%,(?'<Qyv6ß?šPòÔ˜?‹!
Édú?ƒ҈·ÂÏ?ì<Ø8™W2?¾tԗ‹;L?uUy0¦ç?Ü©'ÆÕÕ?¼Ãæ§Çã7?½ãXÙ¤»P?ëÅú`·Xz?§¢¥Œ
¶?°C¶Ú['?¡'þ4ìœ?±Œv #Ô?Ÿ™âÔEóò?ì­Þrf¤Ð?•Ÿ6€^xö?‡'E['Fg?i~îén?·¬#¿4Ï9?"l5Rõ?îî¦]Å?›I-°@ö?"LE5»º?'™Rû9A¡?˜ÜðQ#n?þ…LG»²?çSËÚŸŒ?Ê°<h'?‹ˆÍÓäÂX?•³‰ïRiÌ?Ð|!Üý$6?Ê^út®[P?êW¬®c?°Az^?üD?¶X´h{4A?§ª½YAƒ¼?¶éæ#þz?£'L
{?é99?šRZ?©ƒ³ÍN1N?•¥Áß͟I?ÑUv?ÈfbƯãn?¨ÕÏGZÅAGN4FGL J0841.3+7053?â??dm	@A6T´:çÀ7ÃÜ«g!wÀ;ÁˆÛt´@±'!PÔ@2R¯')?"r×
•ž?͛¿«Q'@,2'1ìV@ Aa*½Bì¿Ô'Õ…-%þ¿å¦BWéK¿ëƇÙ}µ8¿íTÞ긿íäÓôß:Ž¿ïï ×{|xAGNFSRQ3FGL J0841.4+70534C +71.07?äÙ9«š‰?Ñ!•RZ?Õɪh?Ðò@лÕë?€¹y'o?"Ä¢b¿2?íïl¦q?º)}kªaØ?ž¬3߇bÖ?´©[Z¼¢?¡¹5¶Þ2'?§Ó þò¸?æQ…G
kà?´Œ%nc0?É¡ÓY®Çÿ?±à¬9Å£­?º0/7?«ƒP]ä­V?ï:ìÄ ?•%Å~¨;C?"Á:TVó?'õc%¡i?oï1GÀôÕ?s
‹ÁX<:?å9"䣃?Ìd-.¿ä?Õ,jŽ‹–?Ì.º2kb$?£sPœ]?"¹†nЊu?鈻¨"w?Ìê{Z$ŸÙ?¾ûú™±
÷?É	TCפ?´¾-QxÁÓ?¶¦¼gBè?梣Ô%Y?¸Ò§FY?Äô›?X|æ?®ýBX¼›?À€Õp'í·?³"w®Ä@e?숥»tá?±'ÿòY?·P†óL?¯|uñn£¿?'©0"Û9ƒ?é'FLíAGN4FGL J0842.3-6053?í1_ÎÇ£ÃÀ&µÅäêÑÀ9P—2·qÀ<§z¡‡@*#ô&@ºÚâ9Eœ?±j=¶nçi?¸HçÐ^QÅ@1düÙÚÒ@U"–Ó?ïm­íät‰¿à/Z`ž¦I¿åt"狕¿â"ӟNå@¿åbUË
¯ì¿ïÿÑÜ×AGNbcu3FGL J0842.0-6055PMN J0842-6053?ﹺÄ6¦/?šHC<u:?@ˆ1¹c7p?;yKÉ	?€ˆËÑ/I"?š:3žE
?ï–ÑŠO?'ÁÆH3?FRÂÓÆ|¤?YY¤PŸ²:?‰ŸŠÔ—¸?o?³15Ñ??¿'.?NtŸ?`~[ùƘ?a7.‡8É?‰¹™[:¥?€ r¿¤Àö?ïºìCEá?Z—lƒ¹ðë?cd0µ'£?C]úe?x×Æu!đ?W
‹X40Ì?ï‹9:oxÅ?ý±a°uÞ?Sýjጭ¼?VàÛïtØr?Š²—ý?Û¶äG?ï
,²ÕC®?£¢ª;1Â5?ZŽº/ ³h?lš÷–"?œ±~¥±?¢Û¼Lù2?ï6PWf?Š@Ie1…?l	–u¨ô?mH³H§n°?•´Ò& J/?‡³¬•IÓ´?ïG´Üè?w¶™#ü˜?{iõzµ¯?b:ƒRëh?5Œ/E
?t)éìkñ9AGN4FGL J0842.5+0251¿éóú3ô_t@9é™þCg^À;$r[UÀ<©F<û3@ @Öí7%†?þJÅ 0!?Ó͝aûÁ?¹%OšÇìé?á8À ý@VJyö¼
?ï')}§ËŒ¿ïH_	B?Þs[Ao6¿ßf'd@ò9¿ââÒÞßM¿Òä\Xp"AGNbll1FGL J0842.2+0251NVSS J084225+025251?ïÝK;¬mK?_9@Ô^¤?2:.•zO?5˜ˆÉ?p6¿]78‡?^~s#"Sç?ï¡E>ÅÚã?"±äe±õ?[Çvó3?c¡úY)"\?"5Í"|â?Ã7X'?ïb²"¯½?Á)™—?YLóô
?A#"Ø?'†Ø¯€¢?KXÊm¶5?ïUTÀC?oˆˆU¶Ð?T'$ ïm?;L{Ùې'?"
E°/Õ}?n¥ŽÑ²q?ï·mސK?rΙ.Óe¸??BÌtœ?/è´½°a?*r	QÌG?r{ƒŠ÷?ï'ɜ…v?˜Y¾âk?go	Q»?x³1ʘ4(?˜ëM/LŽ?•—äêy%É?îÇtä¥Ü?ÏwïGB?aj0œ¢a?PMñpâ='?¢r€}ä"?AÎ2{Èæ?î$ÄmWÇ<?'!ˆgud?`[L'sð?T>´ÁÌ<Q?¬®hM#þ?öK­DʟAGN4FGL J0842.7+6656¿ì>úz–/h@AÎa(9.À;]u&ÊÀ<›ÚGÓ
@!®â‹ÐÙ!?ÿ`›KJ.?¼_ÿ™þ™N¿¯ž
œ µ?ðçáuÑ@\.Ìò¡¿â%NÂR ¿è8BÒ§®¿Å›
bE'¿æ½™Þ¸Ý'¿Ð'xB±ÖQ?ŒâèÂAGNbllTXS 0838+671?^õPF?¯#%©DÎ?NHb
…›
?AY
pú¶Ý?ˆ÷â$Læc?¯*ðn'…?ï"H\Jv?‰yº<b˜?d^€¤º8è?iM'ã¬?‰ÖHß]lC?…¦C(?ï!,MÄa¢?Šu!âí?_;{=5Z?R|´aÁ?™æŐ¬v?Š;î%‰'Á?ï
ƒ>ìØd?†;ƒ€<K?Z*†ÖdKg?H'Ó0"Ë?ïµV¤Ø?†'=º/B?ïe r*-À?ˆÆ|¾¦ö?cp5Ë}'3?Wñ—'Ä?íêø³Í?‡'_@
¼?îâŸá˜´?¡?
oÚ(a?n o}çŽ{?{Ö«Ý»ÊØ?Ÿ×õé´`±?Ÿ{Záš\?îl»Zg2?"Ž%ÎïÝ?i…9¤2B&?ggïLó?§¥Ð±J¸?'ĵÒ	w£?ìœ1=T?¦ìµ:'üÆ?x†ð7˟V?rYáÕhîÔ?½""=m?§R½¯Pú"AGN4FGL J0843.0-0853¿ã[€Ñ™@3ó)¡¹ù‹À:æž&Ç&À<ƒZ­ËÆ@0]^*Ü@^/æw˜¾?Ò'Y
]Q?ßëSàý±F@p¬bÉù´@	Jod綿Î<x{í?ßÅí οæµùìÀˆ¿ëÇ(}͋9¿£ CX´¿ïýè˜Û-¹AGNbcuPMN J0843-0848?ïŔl3/?œ!
gÝ?Wè/'¶nÆ?['æ|?N?w;½ïÜë­?œ†M{LÁ?ï'-\.ª
?"üL)>á¿?sÿžˆ¥+L?ƒU´ëÄ.¥?…tÙ°ZÝ9?ˆO¾?|~?ïÝü[A?ªNà@?"U½³E?"KÃ÷ó?•Yaê,Žf?‡A8YF?慨Ò'?fºVÞ)?`»2³Ü<?P¡Mö‹•¨?¡~à›¹Â?c6ZVL
Å?ï—..ÞÝ?'ïöÞqL?shœéù?w*ƒúú®?€€pÀiâ|?x¸E÷qP?l'¬¨?¬fÁ«žŽ?ˆ:ÓTj)?ž¤³ÇûÔ8?œuÚ?Ÿ¯õ.Hpe?îIÓf]5?˜–f¦€œ?'WÚúi?ŽÌµñV(ˆ?¢##
Ô²}?'Ìç­Vm~?îËê•Só?‰ÝÕ('?|ï´¼l[?tl&¿ëfŽ?ŸFÀ(°•?…6uþvøaAGN4FGL J0844.2+5312¿½[ÚeØ@C÷…À9v}¾qÀ7À<QU>S"@×Àvþ?ÿðU2a|?ªß™ƒX?£¬Ð6f?ö²³"&k@NFæ™Q ?ï®Ê榓¿ßM™æÆs¿ãN4 C€¿Ö ËQ¢Š¿ä¹ø´²#Ô¿é6ÈééAGNbll3FGL J0843.9+5311NVSS J084411+531250?ïðkrêó?Uƒ´¯†?6‹æîŠä1?-‰"uŽ5?Y†ÿ–T<?Rz90;Ñ?ïÙ~/Ÿ™¨?oób ;ù?FœÊ}ž…¡?PÇQrź?pmO{›N?iŸ"{fĀ?ïÂeâvÆö?p*Ëâe"?VÈ°Š+O?cþÄ0èöd?yL¨H.P?i~ÂÂö?ïÓý¢ÉÞ?R.*-ýž?]iz+Û??CXò/W?mN4<±ÚÙ?KsS!ì>?ïÞ߬M{^?{ÅëÊÒkY?DÖ½À+0?B!ÜÒeß&?kê¤g•Ü?z((KLQa?ï–Xџ¼Á?†€†6á±?X‰ÕD(C?cXîÖÒR$?‡h:l†'¶?ƒ÷†ðh–?ïœ5\
ö?zŽ¦ÐԎK?ZSRé3?]·
Ä°BÛ?…³Ðgç
ù?y ³(‰Õ?gYDY?oÜÿ-ÊÎþ?rÊË	ê?]ˆ°Žåv?tß½J¼Ò?f4ÿ`rÑAGN4FGL J0844.9-5458¿á+€({ÁÀÿ«–òmÀ8Û}½›¢À;›ñþµ}%@|"©¶Æ@7G"ê?©b}=µÌ?¸?ëÓME@§,å;Xœ@¼ÓüìÐ"?èJB1}ѿڅ]à0¿áT¬?8¥
¿Þ_œ}y¨c¿äñÿ¦™¿é̪ÍÛÁAGNbll3FGL J0845.1-5458PMN J0845-5458?êaŽª-?µadž–üi?ïøÞL?ynYŽ4‹K?ÆyZΜt"?´°s#ü¥?èhÚ@Ûy?Â^·)'7º?'wfx`ã?"QŸšnê?Ì
ªç¹{ü?Áˆ8{Ð
¨?íöR0	Ä5?ž [ô€B?†ùˆr$¦?†_8€Â5¯?ªÜzøkL"?šYVìŠ?êçӋ$XF?'71¯sÖ?¢aHýc?vviJ'¼ƒ?¿¿*wÍÂ?ŽþpËak?㐜óQ?ÀÚjÖHݦ?`#-
ì?ƒ;Otüé
?×Ùܔ.å`?ÀyóeVµ³?âU Drd?̼ï¨ûž?¥Ha¹E–?¬Qd@"E?س¶k6"Ì?ËT-
´0?êÜ3ւic?­NÂM?"J‡M?Œ#ý
²E?Â
SË?«·^øõ#ø?å…)n¨&?¢SŠuøR?³˜?Æ,?ÒÓ}ê1O?Ð/‡!qê©?¡"ÉS°&/AGN4FGL J0845.4+0442¿æ>{ÄO-@;lÁ"tŸÀ;OsۙïÀ<§7T*@NI.B^?ÿj`':O‡?Ϫ÷¥h"Ï?ÌûÊ;M?üÿ¦sœ¯Ï@¿P¸TE¿ïÿVø4Y¤?ïõ–àVÂZ¿áúØC""¿ßIMì¿æ¨ëÎE¿ïýøScTcAGNbcuMG1 J084516+0439?ïЄï,aø?cÀÈxÒi7?WZBY×bÙ?Jüþ¹=?qæ÷Ä:ãœ?_Ö_ÇIs?ïÅã¤Þ$?v¢÷‹Ç.â?TZ"ќË?Z³y#ãK?x]é[ë?r%Id?ï'DQØS­?x'©æ˜Ö?cÖ»ò?X€\Ë!(?Šy:ÛF'Þ?v­l\®Y?ï4OÙÃ;?pî;¸¨¥?y"å·ÈÇ?W
üukmà?"ËPâä?oõUˆ™ÖN?ï§áç‰?s¨èg@*?dagû?Wã,ñ‹Ú?!¹]	='?o÷fÙÉψ?ïaÏ¢Xô¨?ñsJO"x?eh²QdŒH?mLY*VÖR?'õk趁?ŽÆ˜×Ý	!?ïG:žƒÜ?†?û•"–¢?pz8"<Öª?e3ÄJŽ?˜Š€ñì?"äE¯x?îÙÏ$üö?ŠÂv:ß?‰ÛN.‡?q¼
üHå?¨û"¢#œ?‰¦}4SÝAGN4FGL J0845.7-5556¿ïœqº¤ÎxÀ !¼jfÀ:‡;©À<#ú±¦@N§¯ÜÑþ@OIc÷ ]?·hã²°¿†–]¶$ÐÖ?Ï$ô×è?èE`üçi(?ïö€[¯ÿ¿à[7¹ª±¿æ÷a€£~u¿ãtUªV€¿ã}éµí¸¿ÕÁ›ì/>AGNfsrqPMN J0845-5555?è#OŒžù?¹¾Iž¦ì?…UÓÁêÖ?}ºÄ{^^õ?Îd'¯M>?¬€Ú?á¹XZž?Åè‡s&hJ?'Ôv‹0?'"ÒCØg£?Û`œç›žñ?Ŷÿ)°w?츞 H?¢ðáè³uG?Œ@{fÙ?"6>:5L?»²+œø?¡áú<ŽÕ?çà·öPÿ¢?¢²z'{e"?°tI©ÇX'?|'1¶ö?ÈBûRFHå?ŸJô>,•È?ãOSÏ­IF?Å71Úîx™?—¿Ñk>›?–`iϤ?×å[N…I+?ÅGººâ¦?ÐüÏB?Ŭ·®'Š?Ÿ÷"Ë4?©¤""?æ‰È3ò(?ÅI—ðïcG?èW_
ã™ÿ?«´Æ^³9Š?›¸c
Èõ?Ú›j
?Ë+wrRWç?ªG:Å+vY?Ý·'-/Qì?­»^鯕?Â
Q$mH?¥Vj0O?ÙB0SQX/?°íDý»MIXED4FGL J0846.5-2609?'ê•K€Ö@%(:û~'À:ž>Ü´¡]À<)›ûs©@"	ªÎ @jÀÒÄ?ыì\ßÿÚ?Þ&S0/@K}\L11@Àíñ_©?¡©³m¿Ù™·@ôfð¿âm5Þ^s¿ë?nu(¡	¿ïÿöût€?ì.¾ù¥sAGNbcuTXS 0844-259?î2'èQbž?¥°â}¼'ø?œ_qMÌÆÖ?¡1YÐgU?['®æ[?–Ë['(å?é»枞Ö?ÂÄ'6Mð?²ªÐ䨛?°^Ö=Ž–?¿}'ç`¶?¾U±ëӀÏ?êÆ-cs*?ª=<¯/n]?­Z‹è&7?µ4)Ó8?»!Oåã
?¢¤•Xé¼w?è'ýC•´?¢¨£"š>?¼s=—î§F?•Åtž€È?¾üØKc´8?žŒ}úô×?é"'e\j?º
%L.›Ž?¹1­ûe?±æuœ7¤?º-…x"*3?±aøƒu?ß|çßD@?Î,æþ?Ïv¡åöòï?Æùoöž&?ÐÇÇ-ÀFp?Çj½OΖÉ?å«#â»Õ?³ɳÂْ?¾"íÞs?¥"å'ÍiÙ?ÊP}{«Çï?®æ–ä'Ï?ىÊ¢:þ?¯kؤÉú?Ñã®37B•?²Ô4CUJ?Ԓ‡Ä&'m?³Ð®CAGN4FGL J0846.9+4608¿ÒÊ®aI=ƒ@Ce]€ä–îÀ:Ò}qDçÀ<–¦¾EJ@	8NÐóx@Ü{£åLö?ЩoÐrt?Á–ÌR֒?ë¹óêH@qð]J´¿Ö,DA"Š¿â݀y7$¿èÌOÏK,N¿éàkB"#¿ïÿÛ¢¨‹û?ÈXp™ñaAGNfsrqWISE J084734.29+460928.0?ïâ)o²aß?`(A©I?Q4éj:?E»yt3?e<GϏ"I?Z"æ)xH?ï¤ë¤Ô5L?ƒŠÄg—°?b©@Oó?l…ßá#1c?'Æ»ŸØ•?{6Ænñp·?ïh‹ã´¬?ñIœ"ÀS?fLyñj?[šæîžã?*™ûwÔ?~a,­ƒ—?ïÆU3>?X—p¼W?b÷]ŸŽ?E%vÜ?žÑ?sµÑß4q4?R@v­ÓWÁ?ïÂ~.¦}û?tKtã£É3?['‹•6ë?U¼ƒ¨:W?w÷È#jG?r"›å?îä™ÓâPÿ?¨dð
Í£?r¤·U|i?€¡pTJ?žêœZWÿ	?§	b¾áޟ?î¸nÆÝ?Ž®ðØj›Ç?v¸˜ç²Ì/?pʇgXÏÞ? ýeô`"?‹¾Ž'pO?ïNhjƒË?|iAve·"?x)dOMV³?e©Öf#?(™£Àê
?v…\%
äAAGN4FGL J0847.0-2336¿íSu̜ @(hïܜM©À9×u;À;Þv˜Ñ @©lut ?ÿ
ÈÅ×F?§øä?'›Ú¶š?ì[?pé!@ƒÃŽ?ïÔv_î¿ÓŠ¬–Ì_À¿áGOµIùH¿Ý¹IbI¡4¿ÙËÿ€>T¿âØÄL0ZAGNbcu3FGL J0846.9-2336PMN J0847-2337?îùÏ.l?"h–ô!D?cñ'nnÅs?X
ñÁêî»?žGéô[ú*?'ŒUvD£ö?ït#M"e?—-žd?[TR°ƒ˜_?iá×åFx°?u,ãôí¹?–jĬÞ>?î©®`aOâ?"È] pÙ?tä«L\Â~?r8ãKi_ë?¢È"3n‹?'@U'DL?î 6ù|ê?€a–†áNn?|[«D5?`æAɔ*?¢
¨S?|›IpÂü?í'ÐàÝÑ?¨pp²f?xɎX‰3?og12?&ã?²\hi¦?§‡¿ò0Ïû?îv2RÒN±?°ÕäNæÆ]?ql#*+Áˆ?'Œêèj'?¦oVlKÂF?®§°¿˜4?í@ŒY?¤àÀþ"?k^¶*\=?}ÞW·=˜¹?´â%¾ÍÓ?£XÆä­?ìÍ«j¸–Æ?š_DZà?'ÍvÇ°Î×?yڅ=0Rÿ?´ßFù*ý?—[kVRV–AGN4FGL J0847.2+1134¿Ð%Pʦ_ƒ@>æãK"SÀ9꣩½ÔÀ<#¥©rU@ þy{Añ?û4<G®ë?´Å"Z‰?£"ö>,­Õ?ò7g«
f@ÀÞöÅð¿ï½µ¢ä›ö?ïþi'jÑ/¿×JC˜e¿Ü¯ÎD¬¿ÝXÏå[?ŸÐňhwkAGNbll3FGL J0847.1+1134RX J0847.1+1133?ïޕ3zÎ?kÁ2=«Žd?E™Ø)´q?4Ä¥LZk?l*¥÷Ê0?jÞÛ³"—?ïÛ6!z#2?r…ê1Vû?H½úà•?S…ŒâÓº?nš›sϵ©?mIYˆê?ï›`†ÜX?wÚ
éQÝ?XèÛ+ûR'?V™Ôì"?†
Âæ>ïÇ?tÕg&0š?ï+Ôf
þ?p$·7kÔs?lÓÚâ,ç?Mš<}óï{?–ë[rž?nŽšU_çŸ?ïÆj»"G#?m¤¾0<áÅ?VaHèLÀ-?N¢R €?w2Pg†‡?j:è£íÅ?ï—)Õfy\?‡p,…;‹?YWu­å)³?có¶Çƒ?‡
›à&ãó?"LÕ×q›@?ï9Ri"S?‡'en›sv?eñ¿[±<à?fP2iy3?–zã#ø?†''Õ ¦?î´YäLñ?‡'ê\}úð?~WÕ_³'?dŸIJ'á?ªÒÏc]¦?†)oÑNZºAGN4FGL J0847.9-0702?Ó\Áع%a@5ø`»+º™À:xºüÀ°À<dÂI¼´@úc"9:ß@°;#Â|è?¶ù¥rë¯ç? @½+ç\?çÏAò×s@ÁÔÜ:Óæ?Í>^!"¿×¦Gݏ<ɿ凾s˜©¿áè<à8Ï¿ä ©¡Nš¿âÎ÷IxAGNbll3FGL J0846.7-0651TXS 0845-068?ᄎ#ìˆ?f·G¸z?W#9õmv?B	Nì'´ð?zÚ);?dÕ½=6?ïÐrBìl?t3#¯b$?Py'Ÿ†a'?ZH"^\?s¨®â
‰Œ?nŽ÷ $>?ïn3#îǞ?,	‡ãA?ioÌjI|?f1rnRˆ)?ŽCécÜH?{#q°W²U?k×`ò?b¤n§°
-?uIeOð?PX쮅ëð?"Ò@Iß+¦?\®œÇ‰´z?ïb°Õ(«?€&ã†$È?l–xKnÿï?Xã™ZÃÅ?XBG‰?}Øn
[ï?ïe"d¯	Ì?ŽF
€q)Ž?iAüš´è{?rµZ#9Ñj?%3ÒP«z?ˆiLhÇa?îŨ=Úà?Š;TUG?z¨¸b]ö\?sâ
k§º? PeÎÙ@?‰äU	Ð=?î´ë~¶
á?NP':ãš?Œ^ú\3$?lÒé—>è¡?›S`²ïÂJ?x8ÄÈ–FAGN4FGL J0848.0-0524?ïG>à1ü@6ÛíúCþ]À:À›f"À<cþë-
$@5?Ìt@3i3 @}?ƀB¸â4?¿v
xc"ù?ô¢ŸÒ˜¾¨@Ô
UÓò?ï-©¼&Œ\¿é¥Œ#Wô¿æOÿAi+é¿ï*Ú~çÆ¿ï¡3Œ†Ô¿åT/aíZâAGNfsrqPKS 0845-051?ïØÐý]¹?q
¶‰ÚØÖ?RҐ;ØÛ?Vc½çÇ?mƤÄ	ú"?müÁ3GõG?ïVö¢ÅMŽ?oIÄ,/Ø?y›¾~#?€Ê'À‰(¥?tˆÁnŒ?"cÇ]s¹æ?ï
ÅsoÁâ?‰ÌéZ՗)?pò‹U盹?m™üÈì?š
®½iÃÃ?ˆh毈)–?ïYO¹Éf?q˜rö'+?"ãÀYít?jí4ó-?"ÈûÛ"èó?aü\~{q?ï«Á° ,—?ƒ¶š5<Ï?kû´¶ò?qDm:h?|!M'!5?~Øb¿?î"7/þ1?¬¦7ØK•‡?'–hY'0?¡@Ix^ƒ?¥x_í?¡íò¯‡?íúfzª¸r?–ÊÛ.Z'?NBL…S?z£¢óé¨ò?¬¿² 
?•Îr†ˆ¯?îĚ=Z?'sîЇáC?¨‰õ­XÎ?Šéa?Ÿþâ»Ïãþ?ƒ¶ïüãÒAGN4FGL J0848.7+0508¿æy
Éî²@<Zþ`Ï6À;U$H¸À<xæÞÆÊT@"øàå³x"?ù·Ab ß?ÙC«QÎ?Á"¼:-x^?ð:CȬ¬œ@ߢ8y™¿ã^V݇Z'?ïƒ}ÎaøC¿èåÛ&+ã´¿á:À›;/¿Ë¡£é©§Y?ÉqŸÕrã¢AGNbll1FGL J0848.6+0504SDSS J084839.66+050617.8?	<È;?…ŽŽÌס¢?F©žY1?@:Îޒf?ŒlcÒù'Æ?…*›ÓéHD?ï_éǚÖ?—fÒûm§¬?hm±ÿÙùã?sXw\b?õ'¯¨kó?"ä)U{ìç?ï"×äê2?‹‰—^z
'?^R³TŸú?c˜Âj¹?™¿ãáE·?ŠîÓ¥kû?î Ù$°?—˜P.Ʊ?b»ö—?T¸.'eQ?¬þ20ºï?—*‡Þ«#?îØÐU[~?š(3r?°?Y"*9O…?XxœEÞÃ?¡¦Y\Çê?™Rò[˯v?î¥É÷m?©«÷®çxd?v@®Zî¦x?…4XbœÌ7?¢åý THØ?§tx÷ÞT|?îP#¸Uƒ?–z3Ø­<?hsíâÂê?oìހ¢~z?©vˆ( 5ª?•þaßúà?ê	vÅ?uó?²‰¬Ý0W?sóŠNŽ^?t÷Øä:+:?Ç:Œ‡§ ?²K¤.5,AGN4FGL J0848.7+7017?ìg—á*@A—Ô{í·(À:£`ó_ލÀ<½ùŸ"®ž@ 
ÜkÒ6?ýDãü";?ŞÜÏyOw?ÍvBýU«®@ÄÛÄ·T–?ÿȃßÈýà?•¬g@o˄¿æŒKgÝ^ë¿Ø'(üùe\¿×m›¤`Çì¿âƁY0ô¿ïÿxPsµÚAGNbll3FGL J0848.5+7018GB6 J0848+7017?ï'tjËè?­¡ ±kÒ?zÿYR]¯?­±<,
÷{?|Fqà·J8?r(+ƒîŒè?ï/®#>sƒ?'ü¸G»ž?|«ò·@?K‹׸}?"К#ç˜?‡í23^J?ï2s­N`?†O¼£+`"?}QTȺ‡'?|7ßßÁ?']GÒÔ-&?gNî'Ü?îX'Y	?"XÞ'»o?˜[JNcØp?rý+h|SØ?¢lÙ¢<8<?*
3 ?ïPµÜè›,?däæø?Õ.ëÜϨ?txÝFúˆÅ?‹çñOêÍ4?†÷UöýXù?í¦Ÿ×ÔÆI?¨nÀ/¹Ó?•z[›<?––¤Žî"}?«ES.@Ô?¡0C·âE_?Nå|'?"íçoRƒ?ˆõ"&è?…šwÂ? .}²V€ ?‹=M\aý6?ëíûŠi??œ8ó'.?¬Šóø	á?à¾ë9~º?¸Ë—B½š?˜Þ=xá‡'AGN4FGL J0848.9+0205?äMˆr9@:îU7«À;(&x9́À<'IÅEïÎ@sñÀ¢@"ę?ÔÀü§…ë?Ån"›þ£´?ó?ª¥Z—ü?íqlŠ†·?ïøgºú<r?Պt";¿¿åüfîK¢–¿àÇ&/>±ì¿ïè5sS¿çåÇ°å;AGNbllPMN J0849+0206?ïRVl¦Ð?›S<ˆb?û|±×ì?}V‡zúô[?–6Öâ)?—ß̑};?í,H5$á?®Ù%¥Êã?¦%J
,?¥ 
Åô!?§iKc¤Â?¡b–î×T?í°!1Q
?ž°[€mô[?'ºo°šš©?háÇ®öe?¬ µ^ä?™ˆíígÉ?ê5SyÇ?ŸÝ@àè?¹H¬E›¶?™eW(Îì?µYSì+Ü?C*`Ì'?íüGõ?»4?¤X‡ºû½?'žO¯íM^?'P?åF‹î?¦ìXÑyñ
? õsBĀ
?èžÞy¿Öç?Äö~G¿Ã`?À˜ÌŒ'|?ÁúŒr-ˆ¾?ºïژèCÌ?¯?÷åõÕ¿?ìXH°6Ù?¦ü"àT2?Ÿ]Lr…"»?"P˜¬†F±?·ênðŒ?£‡|ðóF?åLlû´to?°dí'm"ÿ?Ãd¨ƒ
Þ\?°}ãf´mo?Çi£Ž Oè?¤ç/;1AGN4FGL J0849.1+6607¿Òэ{ÔÛ@B7•=êFZÀ9î.C	jÀ<}Œ†‹ŸÜ@qd<ëmÍ?þӀ*\ÊÜ?³7çßï?£Ê© ¼'\?ñpÄÃéÏ<@	B6n&#U?ïýå^0´¿ß¿ziR©ñ¿â"~§¥Ì¿×™ÒduÄ¿á‡.'ŸW¿Ý×åÐDAGNbll3FGL J0849.1+6607GB6 J0848+6605?ï¼k·oS±?žMʪø?{ɱ$?žQæÔ?DÕ?[mBP?HTŽžÓ
?ïÝg‹ªn?p6ʧŽÛ?D¿—‰ l?PÔÈó½4?m½²2•¨?j+(£¾ZÌ?︾2³º
?o¦y,æ×?WòÖ¦ß5,?`÷ýðã¯Ì?}¤0ÿÚÉÃ?hkôLÇô–?ï«Y¤OïÆ?\ȁjÏé?hmU)èZÂ?D»lòôÑ?~ƒ&ç#©?XMS][¹?ïÛÎdsêU?kšmFWçÃ?Z$¯;´7ˆ?hÌÙ¢÷"û?gD,†ü?V²tŸú²¿?B~]\?…W<"3lø?W(äµ×©Ô?bˆViê?‡sRË
‹Ø?'¼Z»l»?ï‹/æør?xªϸaË?]YÕ¥œÞ?Y»é»Fá?‰ˆÖ>?Ê©?wmÇ|€'?ï.Bç
ô?z`·ÂýÕ©?€ÄfX½D?c[ìP§ã‹?"Ø/ij ß?váÊZ¹}AGN4FGL J0849.4-2911?ÓX(+ö²@"nf¼˜¢À:¼i¨:FÀ<=MéDÓ@Ï`¾1@heD'w?»@DÔn?³ëÉ(]±?ú
üÈ=@|U\'ô?ïþ!8^ì¿åt ñ|¯~¿ß¢ûB+¿ÞžÔw
þ¿àG†Â&€¿ëˆô›GïƒAGNbcu3FGL J0849.5-2912NVSS J084922-291149?ïºw=öí?‡(âs?=J´Kҍ?AXò^Áï¤?€wæSÏ"?‡m¶¢úý?îªcåÇ^h?­Çá_
Ô?X:eDf!?ep¸Ó‡XO?¤—îy¾ß"?­þ%ŠS+?ï
Á.ˆÿ?ŽoÈé'Y?ifÊ;Q(?g˜"è䍺?›'—ákfí?9¾@+¹ù?ïœÍ¡ð…?^çÜÿ:)?ZÂMÍ?5ãX=Òs(?…tMØñ‹X?\öºIT?ɯ6?|ší±e¿€?Ok·W?M}ͱ\W'?Š§m5Æ2?{Œbބ?ì£ý¢Ïð?¼v‰°S«Š?e@Ö¢¢ Ž?}vhEwî?º64s;?¼—yózÐ?î/۞æy`?—>t…®
?sOv5•{æ?rÔê³ÖœZ?ª˜WL³†?–7ºöŠ?îòWi{ø?zÆEҙ^?qS7A®Ò?TØ)ô^?iGH<O?yɐ"!´AGN4FGL J0849.5+0456¿ì5ùø0K@<pÊ>}QÀ9×KÞ$ãåÀ<#)è0Öb@‹v9@îš|îh?¸æg¨…ŧ?¼ªŠ,¿%Å@ዻŠ…*@ÜÁ]Wõ?î™dÀsøö¿ßÈy`¿'¿ß"C")m¿ÙDÜޒȿéA¢a¿7¹¿Ûlk"¸¼ AGNbll3FGL J0849.3+0458TXS 0846+051?ïfq-a.'?€9>=é÷«?w\Z׌?k'|qš?ŠµlS¨X*?xY&v"á?îètpjKM?šG9¢YÆ?‡î§)V?Špýoâ#?–úlnóe®?ì2.*©°?ï'7ˆ=·Ø?ŠI'Øø!?}Õbt °?€Q|×d}õ?"£¶_eý?'©Qoθ?ìÔ9¹ÆF?…eRÔ´ï?Ÿ¬ü8Op¹?u?Ôkþ†þ?±ró%qÁž?RmvØ#ð?î,r 'ö?˜»A+Éß?–Öãe»R?Š$%èáš(?¢.ÍfÞWû?¸!kؑ?í½²J
?ªV…ýV¶?—ÙÞO£x¸?›ÏéPª×?¬5°ùÎ? ãJcaµc?íá7ºE?›8O¬ÚvÖ?˜¹Küâ?'ÝÓ¢dÕ?¥"ëy>?ÛB"ªŒ@?è"½A?´7iH¤ý?³lvF"u)?R%‡fË?žÏ؉³6?™óškü}jAGN4FGL J0849.8-3541?ï¢Úú¦¾Š@ßãß8	\À9"8½¶¯TÀ;ºƒDÃ~o@X®ýÙà@eø5/?·;F}ù}?ĺ…aÿ#Œ@	ÂJ'k~Ô@Ž–±1ç?é¯,ÅÇ¿á–kðL¿àÈÔ_"8¿åþ†]§¥÷¿ë]Ñ6¾Øî¿Ì[ª
U‹AGNbcu3FGL J0849.9-3540PMN J0849-3541?ïb‹<«ú<?"·æ–	‡·?kSv"êáë?cÐsÜãr?D)›FýF?³1½9(?ïŸþ§T1? Îs%r…?Ppûr¬	Ô?_ðµî™S?œDðvªi;? ?<qnƒ÷?î5ŒV";?˜ÎÀ[¿V?"ü¸¡?¸‰¿t9?£%<CŠëÂ?"pÅ}»?¯éÜ?hq'K6Ƥ?]'ÂÔ9K??ߍ+
«'?‹¸à'C½?f±Vð–ÇR?îü«":VŠ?]mðþ˜<?z(Î_YæÖ?s5©øa#?™àYÝÇ?‹õÍèyÓ5?íjŽ©«?¶®ÁøGÙ?h;!=æ31?Ý.ÏVà?³é±®&Ì?¶]9™ Df?íJ°E‹-#?¢O'½<¿'?žÃ‰ÏnŠ?•Ö¸ä¨Ä?«ó6½3Ê?™fûåþœà?î«sT‹s?†JÜì+l'?s[¥*É?\_{¿};?¢ãTó~:¹?…¡SС>AGN4FGL J0850.0+4855?åØ^Z ¬Ö@C¢õ#-+²À8¬ß½jY:À;åùɅ°@ðI°ù½@Ê]†ÃÔ?¢E!Œ¡?«}~o`z@¤ûÍkX@?X@]é?³­L¿KYñ¿ß^y½±%ý¿ãI_à:gÛ¿ãú*~å8¿å±öQo^¿å8!WnAGNbll3FGL J0850.0+4855GB6 J0850+4855?ïÖqµ5<´?­ct‡{ã?0µÇ•ª$?2êÃëQÙ¶?s»Èáb]|?­e=F‡xÛ?ïÖmc@þ3?oéµ±ƒ?C:8Ðï#?HÕRÎ6¦>?rg&ü€[?l²ÐɧA?ïœ
?Œ:"?"›"€"'1?ZB<ÖïP?_4iHÜ`?…´h|ìÜ?"%5@?ï÷™NÈÄ?3,º?µhç?+Èı £…?ÍêAÛ?J©]êŒX?0v;}ÚG?ïæçhÑ?m÷†æ4ç?2@Eÿi8"?%¿&°ýJÂ?fЎ²¼©Š?m `'ÑÑ1?ï"{¦h?‡›üÆÉ2?V»ÇÝGðå?i-Őæh:?ˆIÆñ·*?ƒ‰‰N"?ïTÇ«Xf|?ŒUäD)ÿ?c~sŠP¥Y?h
»^5?'÷<"u>Ô?Œ9E¢Ê»h?ïîÏk—®?L(Þ9<|Õ?;iuöÂ=~?,Q0èêR?[†Ë,ÙèÂ?H¶ŽzCÞþAGN4FGL J0850.0+5108¿Üþ‡µ	¯@C'û îÙÀ8¼$>úèÀ;üyx'â@æzšÆë@IzŘûå?¢ïÁÄ[D?µC;&x@¸ÁƒÃn@§,_›–¿Üo1CD¿Ý<+)yv¿ä0usI¤¿äûR@ê€è¿æ†é"¬ðŽ¿æðc?jyAGNNLSY13FGL J0849.9+5108SBS 0846+513?ïñc²Ê?JúPãÙö·?9"0¾ì'@?-0Ær'r?Wˆ­!,"»?GTa²Â?ïÛè]¡?tk¡5H"?@êYóÁ¬?IÕÉ$ý+?oÝd²í?sv À*W5?ï¥q|w¨a?'œ÷O]Ý?^iŠ9ª'?^à
àºZ¦?'Öo‹Çª"?€ãa¿-Áö?ïý(–5Œ?'tHòÝ?
û"Br8>ø>'ŒÚ¤?3\¥…¯ï?$	íd4?ïá'ä0ÒÂ?`àdŒx,?<ØÍpꃁ?0žÔlÒj?k=åö¥÷?`1?ì\?<ÜÃ?'3Wɪ(i?U›PíE¿?në.õ!Z?‰æFÒi<?ŽY²ÌQ?ïhLԈǩ?ŠŸy?wˆN?d•Î`;Ï?cä†NN?c«¡g?‰pÇà¡7j?ïùñî"?=tÜ¡?½~ïAUÌ?fG´?G臠Yªñ?;V"bMAGN4FGL J0850.1-1212?ïË_r^õ·@3‡U¼Ê÷
À8w1ÅÀ;Ê+"Ù@y@¹åCç
'@<†™Õ?£3ìk£'?¶tJՑA†@pO'RÑ@ßSŽê"¿ÓW‰ÿ¯~¿àæ¯â[Te¿ã‰»€Hj¿åãZb¢®¿éêk
•ù¿äna|òšAGNfsrq3FGL J0850.2-1214PMN J0850-1213?ïìp0"?UCÞÙ?#
?K"CSDÖ3?AŽ÷Ãñņ?YþþhY"?Oz^{¦?ïÚ%󯏥?qÑä°aÍ?KþSó¥ÃÌ?\rROO•â?nÚwƒçÐ?m$×ÎO-6?ï­_LtUp?€
¥Êþ4?i^Þé?vtŠ…óQ?|ÉR…8,¥?u¶½Q?ïùF?ªdî?0c"®²V?#¶=?a
lŒ?F éöhí?,é7lúƒ?ïÑܡߖÝ?n†h}*—À?U–Q€"?J½º'N^L?q¬*ÓÝÊ?k'ˆúD¿?鱗ÿq9Ô?‡8í‡Ww¶?\i•Õ¶t?pSEÉ/¦?'†
i­À.?"ÒŒ¥ }§?ïY4­Âג?ŽY½U'Ê?{ðƒ?'Ýw·–ª?‹ºÅy¡u"?"ŽUŽÎ?ïñ,€;¤œ?IÔ§"¦–?4ü«OÁ¸?&>%iu´?Xgûó'o?GDÄ錎AGN4FGL J0850.5+3455?ïúk²fÖ4@CHå£]gºÀ:RLƂ/ñÀ<‰I÷šÖ°@ê3ß*b@M~ˆœT?¶ç\20¿"_! í)?Þìì\µ½@[œúø\?ïý!ÿ.Hé¿âP_("ƒˆ¿àö¾È'L¿Þ¨,"mb"¿à"Ã`èM1¿Ò|Óz»ÝçAGNbll3FGL J0850.2+3500RX J0850.5+3455?ïÞ^ô=eL?YsßH?FµW5mW?<}T\9י?kóÅûÈpñ?Vf½%É=û?ïßYq±s?m_àž*d?ADh™õo?MF'"'Ô?lUÏJĊ	?gÉ鎓œü?ï~XÞ=?{€5ÈÎ`W?f" õu?n'†ºJ½^?Šá@dX ÿ?vôu=²Ó¨?ï¸ÞCþæ?YKô²qÉ?b
m !2'?@Ì~ŸÃ¤…?z‹§7lË×?VÞjöÅL?ïēæ¯Õy?j¼òÐɱç?V5—™h·?KÍ\…FÌå?x(¦ ¾Ö?g׀|^—²?ï–ïr`'?†À°QŒ¿?TXìH&ƒ?`;Ì{F$?‡¹KZ[?"`O=XdÁ?ïÇ}­€?‰6ƒ*'?rHÇ]æÔÐ?u‰M"Ýñ?š‹•Ag Å?"òò÷Þ?ï:öuŠ5?v`Ôô<#?wˆhá?Fy?^8#ë(?'¿!$È?t3?Q ¸AGN4FGL J0851.5+5528?Í#wb{äí@CsàâiÀ9ÜE ›€úÀ<Žv3cÛ@|"œT‰ð@]ŒzÍ%¸?²4<ó{b?©ýñõž?õŒSâÖ$@
ð%a¹X|¿±ùiã-¿â¢TˆîP«¿âX._ŽÛпâö²ydp¿ãâÔ}›6¿ç÷Àá‡AGNbll3FGL J0851.8+5531GB6 J0851+5528?ïð)ñkÇ?Mš)ˆ(¦š?5ù…¸XãŒ?8ÞLz?Z-»ÉËÌ?H®ÆzøŸc?ïÛf*'=?o˜j8è²¼?F‰ÚŽž?N?Qó€D¥Í¸?n÷ˆ]G?hö§Ašû?ïÌNR¦ô?bmã0?P•­t?9ªŠÞQ[5?u¸ñjêCP?al!<ð5?ïØ»‰ó";?L¨ò'#dÉ?^Ò» häp?9ÑÿŽÉÕè?gÛ3
jþ?FA³£Ü
÷?ïÛ ‡E7?a¶_°å?EG…ÛÔƒ?8¯êí'Þ?o
'+j µ?`¸¤ùS{?ïŽØÛxâ?†²Y‡op\?Zr/Àµ"?cáxû1­?‰ZáNÄF?ƒ«Ï/2\›?ï¦m{i¾ò?rYð«‰<?[£»g9í?WCjh̘°?'ð)¨'Ü?pOcPÃx!?%zý'?kK¿èT?sîýQ	"ø?Wã–~ŽP½?~Ço舦•?dqwÊèu8AGN4FGL J0851.9-5229?åXÚÕ¬¢éÀ˜e"™‡üÀ9·üjIJÀ;~ðW‹@Ë`V{@ä¬{*C?À"'$17°?ª9Ò?ìÊ/ßÏ @	?âTžgà¿©÷؂ý9Á¿ªK̇,¯‹¿êòÇhýÖ¿Ûçœr<¿äÎý>.¹Ò¿ïÿ¹ß	eYAGNbcuPMN J0851-5228?5ç‡?¨§
fí<?Y¾;Òx1?Sn<j´¿¾?¥×­?W?¨wãâ4ø?혻զ²?°"ßQ5‡?I±t?Vڈe?³ÎÆYé?°eO[2?ìø½ªV;‡?¡ž°jý‹?'·ÑuÐ}?üÀÏKSÒ?³ŒN"6‡?­ä$zú?îÞlwL'«?zʗ*åð?iíJ‹‰t?H5ˆá˅í? zcæ‡È‡?xã'Õâ'?ë'@^aV©?ºla<°à]?t2Êív}ò?q†ÀÌ'ÿ*?Áh/qæ*?º爘s?éþOH4?Â.O–¿?_yë™5¯†?oѺL3‹¦?Ɂë{Iß?ÁáÂÕI•m?ê%wô@?¯©F"Ö¤?°×þÎ	Š?–ÒS'¥ï?ÄEO#˜zO?¬×lÎ_t?í\2°?"Ã?ú#ė?ƒŠ°t³Ða?iÆ\žþº?µ+Éèþo?'Ç´xÜÏhAGN4FGL J0852.2+2834¿¿ëGC,òÊ@B×ÆÁ#À:]ÎpÀ<‹	%B¯¨@üܞ&H@'[··?ÆBèé­?ÂS7Q¥å?úåW¨]»@æèî–v$?ïÉ,«¿æì-_ߎ›¿å
ñáe¿äˆ—³æKú¿ð?ïê
_ÕR­AGNfsrqB2 0849+28?ïR/†Åk?ŠDfIP¥?z>evÀfc?s™Ôçº?ŽT뛘B?†yC&µ[?îß'÷Q?žuVKï ??†ÝÑ	¥ù­?ˆÅß°š¶&?˜¬‹âØÅ?•TÓrׄ?ïNWâü?W\z'¼®?ƒ†Üx~À?'^?ûìhª?–2ÆÎFy«?†áÞ! ô?ïDÑà?t•ä˜b?ƒìˆÚÿ^?hvR-#˜™?Šß/ý~€?hD~›L³H?îO:'øë?Ÿ?AÈóŒ?"Ýéñ?yäBkQ¶?¡ÇZ)éŸ?™'³‰
?í¡¢,?«æ$mºÆú?"%ø«^?™•°{O°?¬g|)Ô?£÷êvr?îía½ª?–¦^XbÞ?LÇÑ1Ù?‰Sð•
u?¦mƒ£Zm?'.£"é"?í¤ëm‡þù?'ܵçǾµ?#+ù´á?†S'8a?§¹'ƒ6?ˆ×~®;$4AGN4FGL J0852.5-5755?Ú5
Cñ' À!	3ã\[KÀ8j$咖pÀ;ÁŸr ¯@uƒ°Ï@J߈'4?¢àÏqì=?¹8Ñ,ØÑ@k"˜€"æ@r'M÷¯¤¿Ùg*±"r¿Ý÷"[nç¿ã·ž'6¦…¿ã¶°@O%'¿ç>Õ]•¿æ²\sž]NAGNbcu3FGL J0852.6-5756PMN J0852-5755?ïŒ
‰é×?{Ó`Îð"?P'']ço?C*ؾ>ç?Ší)Ör{?yœ¨Vȧ
?ïŠG<æ¡p?"|ߘ*?:ˆ
_žc?N¬š@ÿö?Œ™ðOµ;?"?4Ì¥"?ï‹T¢C·:?'4·Ë"{Å?fÒ†Æ]?o",rþ½ô?‡¥"ߊ?€Vݏ™6Ý?ïööõræÛ?7YŒ<?ÄÔDtá?£‹+>,?P•ÈYð",?5¶»€a?îöÞZá'?zùË|xs?Pƒ‰("?Ff~©Š‹? 
þþœ?-{·|½?îˬQ_Ì¢?¬VëF¥úÓ?]g'=X
c?zy˜³šÀ™?¢YþÚ(9Œ?«æ%z˜4…?ïcĤE€N?‹ïqÇ«kL?mucOtÎ.?ug
'eL—?±~+˜ÎÝ?ˆ'>žy¼Õ?ïêR¹á7¾?S%\Öþ¨Š?,Â[êÔÅ?!Ùéå:B£?cá $»[Ã?R0++¨ÖsAGN4FGL J0853.1-3657?h2Ð	á¶Ú@°hÀ9/²Ä
ªÀ;ӆžë2@ ­"Ýõ¿?þüÕ©`à?±upÅ?¯Ql^YR?ü˜.•>Á@ĖóL}¿æ­§"n>ø¿ÛžÔA
aX¿à
fÀÿ91¿Ú-'	'`¿â g߿݋c`wAGNbcu3FGL J0853.0-3654NVSS J085310-365820?î;Ñ?"¶ô?ÏÆ?o¡SèW?^#I…€ð?ªQ%bjL]?"Ø«ìò ?éÅr3¤?¼"Hxš?‡ú!dÆG?©u"ý×?Çl$&·
)?»y3÷Ã	n?웕þb#¿?¢Ž~ÅÚÑ?‰yI6¨ñ?ƒOâ¦0á^?·ô&æ-Lé? âbѪƒ×?ì°?ôjS9?‹õþ…'·¹?"úÜ$žœ?q1ŠœEo?µ?IS÷r?ˆ+=Jva?ë›È0c}±?©ÚÞÿÇye?"ÄÜrÅ
?s£M¥äÑ\?ÀD'v×Å?¨Ùqðº'?âĄv>B?Éù<Ò-#?›1÷ˆû?£úNz·VC?Ú7sæþk?ÉR%ç›/?ê5ŸÝç?©~5±"ö3?¦U%°Ú?4UçM	©?ŵäÓÔ©?¨ƒ–b'$?èy6yR–?¤Á×Øò߁?§õ¶¼ÇY?‰ê^³2ªŸ?ȸ—ሜ?¢‡&¬'AGN4FGL J0854.0+2753¿ìgÞÚÁW@Bóâ?$ØýÀ;þ—ó§,)À<öÀ
¢€@#kȂ»0ÿ¤¢F…‰A?ææPaAcx?ïþÿÝÑ@‹{ɤú@ûëLi»?ã&O?XZŠ¿ïÿßÿY'í?ïöü´>?Áâå¨eå7¿Ñ@Æcüÿš?Ô'»/ìVÖAGNbllSDSS J085410.16+275421.7?ê*õg~G?ÇÚ·Àì`?zi œ'?Žœr°ÚOƒ?ƃ1°¶í?ǽӦ–éL?ï?eq&'m?žŒ¢07t?uTÜG^y`?…Ú¢É$=û?'¾ÌAß	?˜/ûƒ4 ›?ë–ëú~?°gæ4¦ž?ˆì¹½€ž?Š²ÃJ轋?ÀɄBð@?°#¦åfßy?싞!ú·Ó?§¿Ÿ¬qý7??:æі
~?8Ú¬÷<­?»ƒÔ
ƒ¼Ž?§»íÏ£W8?ê´J³5)¶?Ã́|±Y?»JôcøJ?"6ßǯ‰?ÃS ƒ®ã?ÃOZùWg?îw1ë""?­b¤ÙÌa-?yÓ_ò²V?‹Öe-Õpø?¥RuI¬g?ªÕO«£'?ê+ð
‹ì?³ì‹Ã$ÿÕ?ˆÖ¦â¤ÇÂ?ŠþFر¦c?ÅÂÕg¦‡?³· êM"?éٝéñ†ý?¹Í…¦¿ê3?2ŸÒƒ‡?GCæ/6x?Ȑy	3?¹ÐÿÙ֏AGN4FGL J0854.3+4408?çún_rðý@D5~g,À:ÎKUhè!À<œ™ì¥°(@ô-.?÷Æ ÆI%
?Ŭ§¾J~?Ò¹]XJÅ@s]Å­ôš@Æm°Ãi¿ïþÞAê05?ïçè絆_?Òç¦læ³(¿Äbl†»ñ]¿çFm!ÁpοÖ5I£bQAGNbll3FGL J0854.2+4408B3 0850+443?ï*lÏzëÈ?™ˆ‡¾ôÉ ?†¶ƒdlôÇ?'b xèò?Ž®H¯©6?•Ôä>§R?ï­ÏÒ=?ƒÞ¡%ÌÉ?cЛ;²S?p'\.0Â?0%kX@n?{×I‰~?íZGI?º?£öˆmXeJ?­
¶¼£™?Ÿ×k-ÂÓF?¢¥x?ÄË?"L•C™hä?ïàV¹Â{?{éó~gq?€ß&q{éÁ?f‰…ÀÂÕ?—aê^`¼?vy¶æ‹®­?îÆN˜`ÖÒ?žÜɅt½z?'SÅäS¼?ŠjÇzü–+?•ã%,I?™
^-?ïîø4ž\?œä¦`»ý?{´˙]j?‹
"·3gÉ?—• ~žÃ.?"q+NRí?ëj~?mv?«éög®g?¶ƒN ƒßò?§R"Å¡Ã?¬X{Ú%Ã?™e²µ•×?î¹·Nê?'µ=eÆkO?‰õ3ÅÀ™,?|*Š°wt?§à·tÒ¹?'O‰iÿËAGN4FGL J0854.8+2006?ëqQct*@AéÈ!laRÀ7'm¾iÀ;Y'àðp@@Öòj–!@>ü½U`…?"ÏÞF"0q?ª;·²@ºKÛ ¥'@£ñ
ݜ¿Äõ;Uìq¿àÍS‰Ò|¿ãá~ ›¿ãD_÷6ƒ¿æ²¥­Û¿â~25r
AGNBLL3FGL J0854.8+2006OJ 287?ïé¡iq³¢?Tñ,€ü»?@èq5aoC?1ݯ(Äó?b$zÀW?S*ªI$l2?ï®8ìùx?Bl␟?U '¥À3®?c¢Ú1Ü?½²›Ò½ª?Ê"4ì ?ï±0–˜)Ï?ƒ§nîœ?dÝ¡!d?u¼®®Àþ|?} ÅäxŒ?€
#püü?ïóÄÊí??úÀ®%o"?2©½ýå)œ? S–îxJ5?SËú¤ªNˆ?<ô	Ɉ?ï؝D7×!?g÷)àج,?;JX˜Hûr?1^?Ê ?qü¸\YEŒ?gNT"úÏ?ïW
̝ä?˜ªÔnEœ±?a©ƒ»²?sØ<J;Á?'éÎ'zIF?–á)F"ä?ï¯9f±˜?ƒ'á©[¹#?cUÀ»ÄT??sϱ"C?~ÍÜçÁ?€6ñ^çv?ïçí£m>-?UÐìê>À?B0dø‹?4¦vYÔá?cŽ>— ?SûØyŽlVAGN4FGL J0855.4-0714¿êœeûÊ@7hëíúCþÀ:ÒdcVçmÀ<wÃیƒ1@ÑÑ¿¥ÇÐ@…ïbùÊ\?ÌhP ~Ж?Ø*´ÿ¦"Ó@	é{Y<²@!­ûü:N¿ÜÍ<žÁ̔¿Òþ=Áç¿ã¥Í"'± ¿ê9QZe§¿ïúÞ°ô?ïua Va¶AGNbcu3FGL J0855.2-0718PKS 0852-07?íwÁz‰3?¶âvuZӔ? "%Uö?´–)ƒ6IÌ?°ë¨Hø±?§'x;dªÛ?îcªÈ§4s?«‰¡¯á±@?"*ÏÅ!H)?˜Ÿ£/*Ì?Ÿ_×$@[x?¢ï! ª'?í4¯ÎJŒ|? årè¢?›cÖ5£K?{}õš?¯ý͙?šÕ%¸€¢m?îÇlU¾£?ƒé£[0?"¸ÆA?ihSRñÀ%?VrH4?>a&?ê­Êå'GÔ?¹¨mqóbc?Ž':m¿??‡n"¬cp?ÃgœFr*??¹"ÖûÊ?ëû""-É´?¼}IE³?«6½_Õ$K?³õˆv _?²ˆ@^î7?¬°"ð­÷?é¸È!Rœ@?°±«I1†½?°:VÐâª0?Ÿ̪‡
r?Àÿ´  å?ªÈͽ!X÷?ìP?¡ÞÌëç«?™åªÕ†MÅ?†
­5¶Mã?¸²Qhð?žúmY¡fAGN4FGL J0855.9+7144¿çÁMm¤¦Ç@AŸÄ~I±ûÀ:=ʝG¤À<H³B¸u@ñonwØ@§ú D®†?Éæ\Ukl`?Ÿ‹™·Ý¸"?Àe$w®@	"¤èWAÛ¿©…Ðäßh¿âõ°¡š¿èÃÜ-'àB¿ã¡Mø±W&¿ïÿÈ!ÂGŽ?ï÷A)@AGNfsrq3FGL J0855.4+7142GB6 J0856+7146?ïògï†Ý?Jùà¶AÈÖ?B?°ˆœÎ?3 `ÅÏ8?R —Ô¤[?Fl*àöh?ïÅêtÊϔ?{H¾–e?Q¤%îŒõ ?_^"t'ƒh?x¡¼FLÎ?uº«wf®?ïdop¦0V?‡T:BZ¾I?a7¶_)¥?`j†
j?'K™µÚ?‡
A½ue?ïÔª‰#'?UèJ<žEÃ?RÎk ©®?8Po¿Ú´?p÷mé,?S¥ØÁš?ïäØGæYÍ?bo
nÏÃ?R©'%LÖH?JU'é?aÒöçpX?^%Ê
+–ð?ïf—[Tq?'&(ƒÛÏ?`T&Öh?o¨[±¿?'"'Øã?ÿo·HJ?îÈ3†¦^	?"+Ëwò†Ä?q«"DƒÖ¤?s¢l.s?¡GcMώ?'mÒÑëè?ïlïå·?zS5Š-?mfíÕf?\N…Öb‡"?ŸÈ¨gø?w>}Ÿ).ÚAGN4FGL J0856.4-5309¿Ì38bXKÀ3éBNY)À:™ÝLvÑÀ;õP~"Ñ@ "è[ôs@fq%Ý	[?Å%'Abu쿆:¾üpÔ?Ånø_»Q@ÇÔ/‰?éíÊsV8ò¿êѓ ÔÇ¿ç³ß@ñ¿åJZ«¼1¿É24/²u3¿ä3ÝbFF5AGNbcuPMN J0856-5312?èDãù}ô'?»)ru,A?q¾ï35?bµ|íD?Î^£_|N?»²RÛ¼?åݛ3¡:?ÂERÔ}	/?y­òŒ¼÷?…ÝvŽ?Óà«'Þê?ÁÒH$\?ëìĔfv?¤FH@Žû?#8oÚAÎ?t ù{Ö¶î?¾zÒÍ‹"?£¢Äí\?í±¡'pçZ?‹^¥¯åQ?`Q¥à‰øÿ?H8^-ù
€?±ðfF¨Rf?‹gèq˜ôƒ?ܲˆCìúü?Âôåm‹&m?}XUÍÙ"?mU3û;"?ál2|î­?Âÿ°¯­$?ÛÓ¬\aL?ÆÌ$ߎ?s¸Õ¥âÝ?"ƒ¿Óð ?âW¤~qlv?Æ´½þA©?åŽÉÉ?³]ÀeæX?'òєä7?€
ö@>e?Ô¡µTé™ë?²Ëؽé&—?è_oÎçP©?¨^dQ–Ž?x6u÷—À?m$#Ï&¿?ͽW)??¨ŒÊáz
MIXED4FGL J0856.6-1105?ïÏÚpç"@5y*0U2aÀ8‡¶Šk(À;ôv_î@Ì/E½ÏY?ÿ.ÐG«<?¤r(çTã\?±y¾\òt@T©p¨	@
°4–	Â?æ^Å󔷳¿Øuaµ|¤¿àÙàvoÉ¿ß@dtß¿äÜ&$p¿âF•Ew–AGNbll3FGL J0856.7-1105PMN J0856-1105?ï䋊¸*S?bvýY|Þü?=À!8
kÉ?8\.ÍÒ?g¼q])ïš?`'¥¾l1?ï¥ÜÀà°Y?'ŒM…ã¼û?d2T¶b?q±½
b³—?'ƒB>?|/ç	H-?ï±o'p@Á?}Kƒ­ÿx?a,¹°\?p»~'Íb¢?~±ÚO9^?wAtHå¶?ï¯
&â ?wòK ^")?{FâA9?[¡<ŸœSº?—eÄ®Yë?u«ókê®?ï®V^JQø?"ßV•¢Ží?LÌ¯r«8?O—°$°™?' ‹Ÿ»o?"
r,¸Ý¼?ïKKÐ/z?Ÿ"×ùÚ)µ?yÏ\#`e?‡B²<@?™'¿ufØ~?™ÌŠá¶O?ïˆ,‰BUÝ?ˆ©Ý%ãÓõ?i›À±O´™?uÿuñ'·¥?‡í'¾¥†?†	‰›¾š¬?î!½'G?Û?[±»Nu?‰™¼6ùý?q
"Y¾K?§}·Ï…Pò?ŽüLYYi|AGN4FGL J0856.8+2056?ÏdÈõ…[R@BD™÷LÀ9úÑáÃôÀ<<FipÜâ@7"/M>@'q›MÏ?º á!§¼?w(ø¿n?âÏbcøM@H[¦™Ý6¿ïÜô‰u?ìýçՒï¿âå‰\4´=¿â•€/eH¿ÝÝkëáe
¿â\&$pAGNbll3FGL J0856.5+2057TXS 0853+211?ï̗7€A?e0?ñ"'?S9ÔýeÎh?@U9*)Õ£?tå¼$6¿?cyfÑw'?ïÙ%%(ƒ'?rŒ™µÙû8?H\DzÏá?RÅð6ù¯6?paäВgÁ?nT©,Ž?ï}K<¿N	?y|øa?e!0±?`#˜¦å;?‹fh"¾é_?u>…äho?ïdNI}ç?j[Šk™q?v3ãA?VÚß6=H?‹à(oÿŸ?d™[§)?ïïþ™è8?zÛ2{dƒ?hY=®kI?ZªÆèß3v?†ª0½&?w³ÈÑ3ô'?ï5ûÃ
?†Ë_ø(¿>?XÄ¿*Ùb©?cý½—ö
?‰é58F?ƒáß…r¸?îðì­£øÔ?ŒŠžK|w—?tz«ßðª?oΪà,K?œÃ¿KɛÚ?‰{ü×Ï?ϐã?ƒ°`ÿuöº?ˆÌ=ÔJ?q{Ý7Pi? QcÇf
À?€ƒÌªvËAGN4FGL J0856.8+8559?Ø<%{v@=(dŒq"À;c~h»«<À<¾¸‡›jT@·à™³Dæ@'ÉÜW"K?ÎÓw¾RŒ?À*ךOJ?î*Ö7¯™¶@Ň3:•¿ìøžï!‹?ãgc¼gú»?āBJR^¿çw5<滿àÆ7½¯l¿Ú¹9±ÊéAGNbcuNVSS J085740+860344?ïÒ?û˜'3?tl<EÞ?Cëô_?7°p?ӛ(?tbƒ¦'ÏD?sþêä `?ïØí6F/‡?rÒ!X;í?Dô•Á°R…?O…º'Éô?pêÒ-ù$Q?nTëÛÖä?ï`}}·Ä?'…/øÀl?cF2<[ܐ?fñ¨U÷fÕ?'"JÂê?1É0͹?﯈²
%?_ä$nª›µ?UÝçzð°†?@ä›ÙŽt?' ÕXN°?^¤@C2?ï¡(ÿ&Ù?znýó)?T¿8`Ø֛?MAûfÎô?…Ù.ÚÞÞ?xÄ·ä$Ã?ïŽýÞ+ˆ´?…_l~׃?W"+ Y¯¦?dYYXýðK?‰\Cü72?'É€ÖkêY?îÐåþ¢û?pQØe?nÉ0¨ñÓ¦?qWñ"¾y´?¡
´Ü?Ž6d\º°?ï'}²Þ91?€4ä•k¹™?e»Ñ>®áß?WÑ*†³:?˜Xς'I¢?ág_÷AGN4FGL J0857.7+0137?æ=]ĉåÐ@<™;ʸÀ;8ž'7À<‹m{-È@…9C¬Å@tßÔŽ?Î.†¦!è2?Ëõ%Ü]Ž|?úPÞªDâˆ?ö¸Dý?ïðÓÊ¿Ç""FZ¿èˆóß`MH¿ÙeNëž¿ð?ïÿø¨ó©°AGNbllRX J0857.8+0135?î,zÓ
Œ8?¬,ÕÝ'ôø?"ý‹£ ?…_~ØÕ?¨5gxК?ªK+µVÉ?îiüÈèè?² ü_¸Z?àY	?©Pàðª©`? ðð' Ԃ? Í¼8''?ízZ·åÆ? <FŠß?ŸÀ´¾øž™?•z«è‡°'?¨yú#êbV?—<£À26?í"s¢íˆã?¾¥ƒ{?¡å{R-_º?…†'§ïÁ?¤ÓJÇ?ƒŠQi2€Q?íߕùjÔN?ª ŒÆÛÕ?ÈDöÖÁ?ïòŒgŒ?ªB.YÌÓl?¦ý/‰ŒÁ?ê~ÛH¡À–?Áš{p'Ÿ?µ@àá"3?ºŠ5¸ô}Á?¶ÈEXš"?¯ï"»CÀþ?ëqi)9_G?ª+É \&S?©õÍhv?`(8ø&ê?·yÐ5Œ?£Ò9'Õ?èÖSÛc,d?©&ø¢Ÿ™ç?¸ìt¾sÉ?¢ÑŒH?À0v2"ÛL?¡]B­ýéJAGN4FGL J0857.9-1949?ÖNʤ¨@0‡Ò"œ²SÀ9`ây|À<kc%iF@-_«·@'ãt®ÿ?¯©.Zêî?Ÿ¾E†®¹?죦-%Òø@6rÆÆù?ÖÙo]»¿ä¤øÝÌÏQ¿çH/^'\Ž¿åÐZ‹fÐï¿æ…bªð3¿ïÿ‹›ªAGNfsrq3FGL J0858.1-1951PKS 0855-19?ïò>½;E?Qï3©K¥‡?5Ÿv 
¡×?'![#ó3'?V§À»—?PH™>C?ïæíšwºø?jþøNsì?<åL¿Ô="?J`jñ‰ô?eu»»¦ãp?f[f%¡kÊ?ï¥ÍrË4Ø?}Ï¥ø«*™?c$¿@ÚÝ?pZÃÝõE?ÃsyH½?y<Þí?ïêÛòôB¡?Bh½¨§?DªÛ"¯^?&»5:ÌÀ?_ò¬:r ??3ôKQ'[?ïÞóøN?lx'3?FO/h£b?AP!#@h?ky 	Û*?i5±I
?ï¹ý^²_[?Ç*:Ë2?T5"ÕFXS?cƒ¯ç'°¸?}óë¼}|‰?:r—J(?ïkU¡G7ø?'Õ"…Nž?n8è(~"?rÊg>?œ"-  j?€"©¹˜W?ïË
6»?a–YÑf?]LLtPƒ?J;5Â!?s&,qólZ?[ÇÂÚü€AGN4FGL J0858.1+1405?í¼ÎNõº@A.j¨ëF5À:¾ã²Â_ŒÀ<oy¼"€@:ªÆg­ä@y\ã/å¡?ÆŲýî?½Ç;¾G"ÿ?ð"X6ù@±øÀƄ3?îÍÑ–0¿Ï­ò';׿è¥8hýœ¿è®½>¿â%Á?ÐÐh¿ïÿý¡UûŠAGNssrq3C 212?ïЋ128H?j¥#	uB?R}ŸûÎç?HéÝÞPÛu?s5´\j?fÂ!Úø×?ï‹Ñ+¬+?'Ú(GJV
?iðq!dÖ?nÒA—)E×?†»ï`ɺ?{´ß ??ï݉1?‰k2º"·K?ÎÐÞVnk?˜gª[ I?•©±ÄҐ?, Ož×O?ï@(Ê#¥!?qCyðè{ ?'	/°âL?g	W^j?ìž_??fd§TÜ;?ﰆO\V?tÇD
e›{?YNSl†Ž?RcìC¡ž­?€´¡Á1^?rœ»ýd¡Ã?îÆwWÇ´?š	ïµ2ò?|¹uë1Ab?Tè'`¢P? [Æ`ˆ<?•xÒÈL?î\%јL?'××Ò@Rv?‰U­lÆc?ƒ–b¿R9Ø?£è8o$~y?‹ÈÔ39ÿ?íÙA,p y?ë…m¿U~?™KBiI)F?…J3–4©8?¥ÆLYcÆ?"¤Z:÷AGN4FGL J0859.4+6218¿çpøiø[
@CDhۋ¬qÀ:ÀõÄ<ÛSÀ<±‡O:J@4·jºÞä@WdU/?½åœQ"×ì¿}æñˆTC?½ðÆQ2¢•@u3`œ˜?ìžÊÆbO€¿Þ—u;Ê¿èú'`åóå¿×µ£euP¿ç§ÛACl¿Þð?ãÅ·°AGNbll3FGL J0859.1+62191RXS J085930.5+621737?ïçøê.~æ?[Yy²Qc?CÖç¢ á?76ö°ü°?c[Ù*åB?WŸåôs'h?ï݇Ê[¥»?pŽIÑ?Bzû5›?KžèÌ5øm?mò—‰\?kö؏OË?諸HóA‰?w`']\"?TˆéBZu?C}[µ˜?ƒFP¯5†K?v¨Ê,Ñã?ïÙ4?³ÛJ?L"âpC4É?UÕǜ0'³?6•+Ânً?kàÜ£(iy?GïSìjX?ïÎӖŒì?p y–Å?TÇQ^X,?GÄޅç‰?sÌP2§æ?lüxz$à:?Øg¾3?"[ßĵö?Q 6²ÚS?\HE¡dè?†oåýú?'I=Rõ/?ïU5_nŒ?…(Z ¹²4?`!ƺì%?^­Xsúš±?"[~@|ç?"nnZð9?¬4HS?oVUǾf?rsæÅn?ZÐÛå†a?†a–œ.â?iØÎXØ$?AGN4FGL J0859.4+8345¿îîxð{@>MÊ:KUiÀ<êäåÈFÀ=5ôÆ/@"˗‹!†¸?ö¾0'}ó?Õª• Õ`?юcpàÓ?÷ÄÉÉMì@ž}"D¿ïÿðÇô ?ïùªæÈ÷U¿ïÿoì÷å?ïþ=BUºó¿Ñ¼§›dõοáñ@ÅÂíAGNbll1RXS J085916.5+834450?ïŒß0‹F?Ž¸ç<º›r?XÞ;ô¿?Y"³{Ø?‰¯ÀB<õÜ?´•WòX˜?ïÙ#3zš•?sÜ­pî?E®Y#?P_A¥Â?p¸£<ê+?pòÈ̏Ì?íµ%ÿC«? #M'â?'7dÀ¨âò?†CDÎ;6ã?°ãnÚH?ž|ˆ1ci?ï¿â'º?l'±¿öe¦?R[	Wu?Lðuµ8O®?{wõë
*?jŸnäôê®?ïGQœ;Ä?'ævµ÷šÂ?nëõ֏?pḜ²Û?"8j|6Ÿ?'iRl??nGœ<?\™WÜã)?qv«ëF?‹[íQu?ŒUï™Ø
0?ìça,ãi?£øû3O~<?‹;ªƒªM?Z™1G~L?µRï$sNm?¢²{çÒä?ﯮ•'?'%—톦"?tÏY€Ã?|ûÇK¢Ñ?˜–F™e˜ë?hËßmâAGN4FGL J0900.6-7408?ïªÔž—.À1úgèF¥×À:1Y³Ð|…À<7ä¼­šØ@~Ë?"@¢ùà0W?Şԁw
þ?ÉhÚÆ_ ?üö*ÿˆ
ü@	}Ð3´f?àbù"«ô¿ä~Áï#9¿ë¦°8Aí¿îg"¾Ái¿ÑAÿE¿ïü-""ÑAGNbcuAT20G J085959-741401?ïï\Çß°³?kCýùE??~)îUÁí?J,t¦½½ê?Yfåå¿j?eåg*µ?ïϼ£´Ð'?}!l
Ó¨ã?N›T-dè?`ߛ$>éÂ?t_šÆE™D?w!"w_~?îÒ£)K?"¯Ê-l<?uŒšûìçt?x¢k½LØõ? $:³u4?'ät€§Ò?ïÏíè²?W±Íè·¬-?Qad&KÀ\??tà_áي?t&°{Wï?T€6Òh,æ?ïÜÏ0Õ4û?s<¹mý?Nµhºg?OŋÃ@÷Ú?kƒtÿZb}?pàÏoà©Ì?ïnä6`'?'øŒ0^ôU?eù—Ôp Ï?veƒêg0Ì?ŽÈŒŒš÷u?q>ßùJ?íȦ§@˜™? ãä'p?ƒñ-Rì/—?ƒûÜá–(8?®yJ6Ž?ž7{ŲÍ?ïcƐPM?y'"äÞ5?l¿¯Õ É?ap¬\2:?'2¥–=?ué0"2AGN4FGL J0900.7-1243¿Ö&
Žf"@5SÂCÜΣÀ:8èí"ÃqÀ<`ÎùͶØ@ßڃïŽ@"'A?ºh…¥pè?˜tŸ¡?ß"äRzv@VÞyzÐ?ïÿÞ§À£Ê¿Êši7Ñþe¿æÀŠt8¿â-%Òø_ù¿é-"BJ'k¿Ú&$"AGNbcuTXS 0858-125?ïèâù2†?ZGêºõe?:ŠDʐ?.Mr¤°lÉ?cÌ«µh¼?X(–LŠ(­?ïæ&G'eÉ?my?Ýì©ê?=Á)ù?i?I/8ðëô³?f6=¢­Ö?iLºþw"?ï_ß¡ï1.?€¡QÔ?b~½¿x"V?iþ˘á`?'´4
Úµª?‹õzÓÌ>‰?ïí,	·þx?AŸó¿ñ˜A?:ð+×hÑ?‹ÿ=L@?^ëáéS;?@E̶߬?ïÖã½|?kï9Œ…3?K§Xö!?@ÿ ¯'¹ƒ?q'*u?i…߆‹á?ï®:50
?"ø¶•XE?PÜÕµ©ò?`kĖ"ÎÑ?'UØ	Mÿæ?'Û>¦/Ÿ?ïîíÞë2?ŽeŠ"?Œ?lþ«Lå'ñ?p¨½á½îº?˜bLۍËS?Œô(RÑÖn?ïËÆÐ3‰š?`*Zj{?RíªE6?;àU»9W?ux\zWɐ?]G¢Ìã8ðAGN4FGL J0901.2+6742¿Þžh3"@B‹kü¨\«À:iTK±¯:À<cۖ"+œ@¥À$Ä!@rü¬Žhä?Ã_5'n·y?Âf‡s|O?üvѵ(@ ov°?ïõ8ü Ïï¿âçí_>~ì¿çÃPýsˆ¹¿ä4ÂI¼´¿ïÿ¤€RuÄ?ä‰áàÛ!¤AGNbll3FGL J0900.0+6754TXS 0856+679?ïxé|A*S?˜Jæ__
?wv ðôÊò?…ÀHlñ¾ö?†
uÛ-Ì?Ž:§S"n?ïIŠ†ö§?‡¼ýjÝ?xiUVc+ü?y×é·Ç^?´YðS"?…[ys?4]L?{íG‡!H¯?g÷‰œõçG?e"­ÇQ?ˆRùÙ­?wÐ/ ,?ïB)é'V?qµ‹—JÄ?'›édŽô?bý1ÉBªþ?ŒÙœ2?j9Dí_\d?îô›¦ö4¶?–sq{h7>?‹æ£íÃWý?‡ãÃínå?"y9(Ÿï:?_3e^ÞÆ?îN:x¹?£1´f¦1•?†fvsÓ ?ŒƒLOã
?¥'Àó§ak?ž$|†ð;ë?îà\…«¿Ñ?'²æüá®?yÑa}¼¢í?y6Ð
iÇa?€æ¡_6?Žœ¡-Y!?íX%û‰›?"6[…? Ú
.?…‹ÿMº?©ü"ok?‹ª}"Ÿ"WAGN4FGL J0901.4+4542?̊4e§˜@DªV"uÀ;É«¸€®À<ï[:¹9r@ù"D›?ü‹rX?á^$Ñq?ï÷ÝâsÓ@$ †å@í?³õ¿áën"cÔ¿ÁÞ/5L½ô?í_«–òm¿æwˆ,‰ËÆ¿ïÿԖũÃ?ç
ò¢IlAGNbllNVSS J090208+454433?ît&ÿ"kE?¡w_±ëi?…Jˆ×'òß?ØBÚÄ©â?£jíÒ´uñ?žµUⵗQ?íFÛ¢ŽÆé?¹R¾Êë?¤èŸ0=ø?°´ú=_‰?¦©¦½Ož|?®'´l1@?ëåOªã?¤oû́­´?©Æ/5°?›Äæ}/?´RÊ?ŸS¿[$\ä?íS•(ƞ?˜¼T.«d?œr	'–ºð?ŒTÛäÃê?¬•áíàª?"'ð‡Rt`?ìbÑ©Þé¸?³ŸÖ"^·¿? E°ð?œ?–Üݛu>?´ÚÏØþ…î?±É˜)
'?é^€ØœR ?ÅÁf–{ƺ?·pÑ#á–?¿²?'ÌÎz?½›(©Èn?·—Î.äð?éy;T-Ãv?­ne"ÜK¯?°Ý»|À'?ŸVÍBó­}?Á¬4í®ªß?§Ž°Ø0 _?ê¼ŗ5?±9•l^.&?¡'ìd_œ?šÔ§"€&?Ã\"¸U¾Æ?¯ý±'GAGN4FGL J0901.5+6711¿ì~V[¯¼@B¥Ÿ<pÊÀ;>Iç«À<Ÿ.X•@ 'è(ó¿*@´{'G–?ÂÝ`t#"¿…ùN'fn–?ÅúöÖ¶…Ž@æ"Ïíú?î'"2wL?Ö"D"™³¿äx7ÿ˧´¿àõ½ò>v]¿Õ¸"þ<[¿Øæþ§:l
AGNbcu1RXS J090140.8+671158?ïÀdÀZ3ä?jü>ø^Ü?Q½Uv*.ø?BþÐ÷3?{^JRÿjP?h—Pøk»(?ï´­Ù "?wÑ¡Î<~?S7ôž…	<?R°º³Ð5?€'•ó¦=?t®jŸM¾?ï[IŸ'Å?yó–ZK°?ZoWk>Ää?AT_Õ´ò?ŒÛB¶|áú?yiˎñá?ïi$ª6þL?qŸœ}M­c?gnlku?N¯pá@?Û:X({˜?qh›s.8?ïx,˜†Á?r̓?cIöZ›8?SsOȵ$?7Q¥å?|7:T;Î?ï]{/Éz?Š…Ò³Û®?\`K)×i?aWà)‰…â?'Š•Kªn?ˆów'zïÊ?ï–ô+i?…Lbìú¹?eÄΓçF?_ð¶Ñ?œô‡¥?"-XW?íøA~¿<…?åDì,ß=?'˜†¼J³?pà@ƒ'2?«úñï1?ä°çßAGN4FGL J0902.4+6440?éÆæY÷ÔI@CàÁvWuÀ;A&"Ï:À<ÂFÊ¿¬S@ǯ½ó@)@ç*໗?Å°'åøý¿ OáGÎ?ÖùDåè¨@ïƃ°¿âëE=¡Ì¿ë'} <5¿Õ1e¾àÆ¿ã¸É_¯èæ¿Ü¬W¿ïü­/x"AGNbcuGB6 J0902+6444?ïФ‡«§Û?lÁS½"iã?MÞ…¤?>$ƒóÅ7?t
€fÚ¹ü?j´Oí­à?ï×Ûs®£l?n,]ď?C¨>dè?N‡è%œØ?q®ñzÁh?i^/‰{+?ïRÂxÇ"O?"m±.Òw?qIæ??y£æqC?'džrîËT?}" hí2«?ï×pÉZ–=?T8ý¢*«[?E}ð»-4?1d&;"?q•ëuj¡p?SLàv¢?ï~¥!4?"[œý´ó©?`¹‡t¢Å
?PT,æñ(m?Œ(Y$.i'?ƒ‰üë½ñš?ïŽÖû'u?Š"rðW(?Suî#˕?[ÓVÐ+‡?¹›"W7?ˆwh¥˜?î½Þ3–IG?Žp¾¤ò¼?y®6†'<k?}¹Ñ­œ+? ìUó	t?ŠþÑê‰o?ï~Ic\'?v6ßk²?^QãÈGõ?Pœ+¶¼f
?Œ©ƒlg¤'?u<Ù-8AGN4FGL J0902.4+2051?éUSî@BàûC؜åÀ8ë+•°À<út¥ÄJ@𗏩*Ü@ã`dÄ¥·?§ŠI€¸³L? Ä©H¹,?ö;ßßÏ@hGn~Ð¿Ò<Àåä¿à5Úã1¿âIšHB‡¿âTä(3$ð¿àF4—·AJ¿éE‡=÷\mAGNbll3FGL J0902.4+2050NVSS J090226+205045?ïów"i·‡?PëšnW?.¬Ofê×l?#ÒpÅ:L¿?U;M]©Çñ?N 6È+I?ïÞA_¬ôü?kmîRÕü&?@²-V%Ùµ?Jމ
ìís?m'<
pê?f×É=¦?ï»ux
i?v¹‹JÄ?[òµî?lǼÏJÕ?{…]¹»ð?qåì|?>£?ïè¥U~Ž?FÀ̝ç?E¸oÞ§g?*Núøô,?aìŽÙ!?CŒÍÞðm?ïéò}ò…T?]tCÇF¥R?:õ#àª|o?4<'¤ˆ?b®ÝÂv.F?YçAð˼¥?ï¡F–M›?"P?šV?RŽ8D?_·»¤£'T?…{nV
¬?'Š‡À¸ã?ïŸê‹=z?xL(þ?[oˆŽ°b®?`_§"Ø?"ÊÔPÙõ?vì5ÐøÒ£?ïËΌ?"?bßÓ.ϗ÷?Y©½=Œ¢@?E8¹ÛA5
?t©hmI~?`>NÖc	ÌAGN4FGL J0902.5-4801?»6í+UÝò¿îÃ"N®ºÀ9 ìt2À:ÞÿÕ8@›ýèx¤×@Q<\§¡?Îãî<Cñ?Üj¹œÄFk@Nªß<;?úi·¬T1[?íD8¿HB¿å¯m@u;¿çÐÓDM¸¿ìŽæbJ"
¿ïÓ±B'±v?Æ4Ü5JAGNbcuPMN J0903-4805?Í¡â,IMì?ÀMJßö9?ŤVzÏÄ?»œE›jª?ãRÞ_Nø"?Å;wqÈç‡?ÇMüÑç?Á¯5&X÷?Àì%¶%Ÿ?´ÈO;ö?æ=qw]üØ?À›n¦%îý?еÑ)'q?±"'Ó¼%?¿¦Q´ŽÎ¡?¦
—¦Ñð¶?ã°M4]¢?³@2""v`?©7×tXˆ?‡@myS?ʔßD7:? ÜË?Ì!?çÇW¡–W	?¢ùb'û7?ÅX炙?¹x%…vì?Â̅›5!?¹=X°Æ0ü?æƹ(?ÂÃæ&î‰ê?¨Äy¾ž;?¯®€äõk/?ÂËV0ŸkQ?¾µò"†%ã?éÀâØ@¸?¿ò˜9%?ÄyÐC­\x?©v–0Õ0?À3²™‰˜?¨_ô~5O?æÔÇÂnF|?²Ö[ގpe?"a[¢Û'.?jàŽêvÓ\?ÍñUz'ZÚ?©²™éÍ?è2%2®Aá?©D""NÖþOTHER4FGL J0903.1+4652¿ï(tJL â@DÉ}ke©¨À9ǽWäÃdÀ<{¬h©6Æ@òS™Z. @üc®%AÙ?¬¸9lÞ$¹¿¤€ýbäC?ö‹‹Ÿe@zêéz¿ÚÙaE?OK¿åÍ:°ÕöA¿ç0[b&eÅ¿åtáTù׿ÞFãÿ™RÍ¿ìàÁvWu2AGNfsrq3FGL J0903.1+4649S4 0859+47?ïÕíÚi?ŒÞÎúEù+?P&$ي¸?ZŽÛ†–5 ?qiéøév?‰Å×%›d?ïΗʃé¦?ŠÛâêEƒ˜?K8+¡‰¬?U–,tΙ?uM-uñT?ŠdŒd|È?˜Yõâ?€'^ûG8k?YL
>Ð#ß?Wº¤+šð?†p˜•ù×?"˜'#ƒß?ïËH6ê;·?X³j'ÓQU?dˆ›tWE?Jvñ3sO?p–Íöé7?Qȓ"èÉ?ïaN36/´?©Å_™cUõ?t:Ûof8?˜ïu {ö?y¹ä?ž.R ƒ:?ïQR@r>"?•´(¸œCa?apŽY[ÓF?hҌ,Þ*N?"§¦*TE?"¬#†ƒA‡?ï&Þ#ž¸?ë3œ§Ð?gÖ
yÎj·?h[òV`•/?˜)z³áž?Ž,{êú7Ô?ïSxßaò?|]2šåԛ?ÂF9áÕH?nÊh|ì¿?‰_´¤,?sÀ"€ñŸ›AGN4FGL J0904.0+2724¿æUÌ",ûŒ@C÷Ä"`À:E®†¨YÀ<|Å<µ'ô@ïIp6t@~*Ã") ?Á—ø¯©¦W?ÆO¬e¤®?ÿ¿ôw5Áƒ@	¹H~?Æ]B Ç¿ç§"™2¿êß"²¿ê§}½›¢¿ïÿÞr¾"¿é´á¾ÌY
AGNbcuB2 0900+27?ïî²Û_Ô?Uu"?À½?PéÙÜâ#?HN[84´U?Q°p>
5'?Lÿñ½Óژ?ïˆ%Ð
ó?ŒbºIol?lï2'¸?s̊ûЪ*?†º¿~çƒá?…?ñ3?ï¬p=ë?t`ùô†ýÆ?eêß; ?^7k?î?zRfµ,Ñ?q¼ÿÀ	-ó?ï'ï) ¾D?fÒ¸FÊi?~+­Íjò?`!H¿'n?xܽgT?WÚ_ŒI{Q?ïޟ	g8?cùý|x=?aa'WÜÖr?YKLÿ"ú"?_þèGãû?YVëgI¦?î¦3V!Ri?¡à¦$j¹?½Íre€i?lE ç?¡-WEU?šÔÖº?ï`/¿z¸?ƒâÑÔC¾?tcPFD?t/wPìD?Â–ÙÐà?ÐâD$?î¨IâŒ?‡Ë–	úÒ/?—羡®Ž?€VŽŸòüp?"¸<՚è?yl2žYèAGN4FGL J0904.5-3513¿Æ̧ç«@<Ù|ÞwðÀ9cЗ\¨À;Ô¯ÂÐʈ@'º.9¤<@¡&cAø?¹VÈ8¾b|?Ä@l³sà@#xà¼mÚ@.="‡¿Ì
#)$çk¿çw9ó@ÔÜ¿ãঋ(¿ë2O¨´¿¿ëÛÞ´UÞ?¤@ª; gAGNbcu3FGL J0904.8-3516NVSS J090442-351423?ï¡2"D¬
?Ž+‰ Ç*?lQv;m?‹ô·³œ5f?€Ÿç®ä¨?tu1¶€?ï"ÍêP®?"«£7
o?H¿Ê) >?X>©?‰€•
`&?"õî˜?ïô¹û¹Ê?·•Àâí?€œg*¹Ã'?€»َ{×?—s5*$ù?ˆzì™ì‡?ïÓ#ÕŒˆ?Tõ¾E9ê?Gòw•.™$?,]Eòõðô?soƗ"'?SM<RÒný?ïH‡Æ]qö?Šb6}€ä?vG–ÇI+ ?qXëUç?']!gÐZ?…ã‰âj??îÇ_Þóüù?«¦a
¶ø?^ï
H¤j?sT`–?¢'‰£åõS?ªþ‰hŒþ?î0ÇÝh•/?˜ÆRÔQ?'#•œ¹þ?Œ­jnÏ9»?£êpbì?"ڐ_K?ï{¡w7?tØE["Ìi?a¾YÑ/mŽ?M¿°â	ˆ?Œ¨¼ª?s¬
lðAGN4FGL J0904.6+4238¿íc3'¹æ@Dø<÷TÀ:Ÿú D®†À<¨¦tsoc@tTc¯|Û@ôóg°?Ä©À˜¶ð˜?ÁǶb}#?úOSû)×?ùA˜‹Ò† ?í@֟^'¿åIÁêñ{¿âpŒû%¥¬¿â}5€V¿äpŽ•·¿ïÿï¿@PAGNfsrq3FGL J0904.3+42404C +42.28?ïŠ]O¼V?"æTœà,?k6,O{?q¹@`ݵ?†­Ý¥5yÍ?€N§-Fƒ?îï7Я?š.Ó?Žz¿éÙZÌ?‰c`¿¶Î?Ÿ¿€© ²?"Ïwo"°?ïMÞ8ô¬ÿ?€­Œý‹?o\éð1z?h\™×T¬ª?'X›§¯¿?|½ìC¢?í¥}lV.?ŒnÍÒ¬?¥AÄʹõ?œTšn#G?ªsã[íW*?'‹ß—‹¿•?îԕQœ'?•G›Ü%A?"Š¤Ê^"?zˆ¡Â?›(n
h?¦‡6í1Y?ëÙÈ:ìºÿ?´Ø•?Nƒ?¤àÓZ-¸?¤K
Ç,š€?¶ÁTž$ß,?°>B?K º¶?X‰FÏ!?€¯Ÿï,?yRͲ-F?¡èô䂛Ý?‹ÐGÓ½ì?èvG™`}ˆ? ò%é"?¸¾Ô³æg?˜‹	31?ÁÇw–mì?jSÀM`ÒAGN4FGL J0904.9-5734?î'²¨xÀ$«>݋aÀ7ÉÜ_çÇ$À;IŠ]ÜT@©b"@Úºp©¶?˜#yç;?¥´t€b0@
6lmçd(@"›æ¥ç¿xÇ!€òól¿â$Ÿä6v¿äFÿ=T<¿ãw÷*|«¿ælŒñ«¿áÛ~ AiAGNbcu3FGL J0904.8-5734PKS 0903-57?ïvßvâNX?®½ØtRª?küD™Âö>?©jñ{¯ƒ?‹I1yÌT?¡=¼«ÅÕ³?ï\;!5§#?œièÂoÓW?:Ï|Æè´/?KÂÂã#p¢?"
]æ¯á?œK8œ?ïc\ã¨'ô?‡šëw^'?lñðböÑ?v³/WßwŽ?ìJôùoK?…&ó÷Ãwb?ïöƳƒ$¸?9؉­"?帞3w	?•«‰?PÄ=+a‡?8ÀԞÿ(À?ï:­zn}"?'û{Åô?DÅÙ¢'Ï[?@þދ˓?˜!Ý&_†?'®vƒÑ›?î%Hu©i4?³A°<÷þ?S—dÄ#}­?i6'É­éÌ?­½€P2Í?³OÇú'<?ïí§+Â?"cŠ{ßîi?s<€ßB?{Ýd4?—³=Ð2Ax?Ýmµ¹U?ïí'?${?Rñ}'v
H?-ZËÂÃN?"gKç&7?aÂ=6 0?Qí$LXAGN4FGL J0905.6+1358?ÆÓá¥2:@AûÚ¾'œÀ9PvÄ À;Ì(Hôe˜@:grÕàr?ùv÷xr¥?²‡›À:m9?Àk.¢)àú@ll—ØÏ:@
õÁòSD ¿Ú½'Æf>¿º{Ýñã1¾¿Óžœ"_ü?¿Ñƒ%Nn"¿àäëa¸VÉ¿ànÀY!AGNbll3FGL J0905.5+1358MG1 J090534+1358?ïëeÍý%?~qLϋ â?Jq®/B¿P?HA8øO§?[ûŽŸt2Û?~
þ0Í_?ïÀ'_ZÐÓ?{?Ͷ±Ì?XYkYo©?bâøýj?y õƒÒ>p?té_Ò?ïªR2
)š?|,?·ò"?iZ|·"eÔ?rk˜òÛÏ?~)¨ª—Ð?rpÅ?…Á?îL숻@?…[UOãy)?xusݺá3?WÓíc¬]þ?¨"ˆûm]?")	®;|'?ïãa²³­'?g]ݔ¼ÙC?V'(qâ¾?Siâ©Ž?a]99Ýj?a¢GâȄº?ï11VWó?—òóŒ†	?q'ï²O%?{i‰,vB?•uc ºo?•å(Û?ï~]Xu·è?†,°}¯ÚÙ?qê'×ôÎ=?|"£ÖwÞ?‡s`.¤Ò?v®j.›?ìŽ@ä1ÿh?¡'¾ƒ*d?†1=Ÿ#Åx?mÜôm"Áê?¸ÇÑ*‹Œ?fÞ¯˜÷mAGN4FGL J0906.2-1707?îïT«°·@3¾G'ܾÀ;"æ>ÚÀ<l»êý9@ x–†>Èé?þ0M:Ev,?ÑÕn'€ñ?È;™¼)<?øääÖ®ÍÞ@4ô‰)^ô?ïÅì=«\:?̵FÞ¶¯)¿£O.D³Å¿Ú>Ù#ó$O¿àœ¨AÓ	'¿ïòË.g˜AGNbcuCRATES J0906-1706?ïÀô<…õÖ?o¶î•–?QGnZyé¾?E߁÷Q‹?{4*†"Y?mVœ0/œ?ïWÂEyÀ?'‡"
ÑF,?nR	¢#­?nW'FK²?'=v÷æÓu?>x¢gÇ?ï];Coc?€:ð6ł?k*I]ù§?hí+•Æ­y?êSQ}úk?{(·?ƒð?.¤¿?…íªÉà?ˆûɤ?jݨ®\¹²?©U³ÖO»&?'Ø̱‹?ï'GÐp'²?'©!l¤RŒ?`™
Þµ	'?V™RJV–?‡‡ÈlÝý5?[è$ê?îO¦r^±?¦ÂŽŒ?ƒð:—­ë?‹»"‡<Àh?¦@ÜÐ6Iú?£ã~¼‰ã¸?îÜ®d+ùƒ?‹ÎÚ"ˆ±Ž?tVôÌ:—?r..[óôÁ?ŸTw¢f?‰»ØÒ¢KZ?ëZü°•3®? µªià?"œÝWÓw?ƒÙor&¬ž?Àq'ÇöØ?Ÿ#«$P"AGN4FGL J0906.3-0905?í'J^Y7æ@8'sÕº²À9óÿò"³À<Qäþú2@]oqÒÖ@^쿱[W?¹*³Éƈ?´sßrkØ?ûåCÃC@‡-ã"ã?ï;ái\æ?¦½nú£¿ÝÞa_@'Q¿âØ)Âq)8¿ç!½T‰Å¿áŽýÉÄڐAGNbll3FGL J0906.3-0906PMN J0906-0905?ï÷æÓ«…¢?<ÞàèH?(¶›ÜWæ?¤›º|%^?J7
kQŸ‹?8ޛ'çæ ?ïæÎDŠã7?k/F-z¦S?=Ù0«›Ö?IÉè6'!??ev•'c•!?f=š†ÓÀ?ï¾°ûhŸ.?r%²ôü1?\FáÛ²Æ?kŒŠßaåÑ?y•ÉÁ¯¬8?eNÏVÎóŠ?ïà]Ãæ°?JÕ9[x:^?OëÉY&?5?2mCžCãê?h°'Sy?G¶PzUoÛ?ïõ ÷Ã×?DBYa™×J?2ó_ì¸D?&'–{¼Ý?PKõ‡Q—?@²ÅkÚƗ?ïµ`àü•Î?wÏÖÕ¬Ë?P"ªw&ðâ?^ñ_œ|[É?€£ri^¨T?~ôd×å?ïžã+D7¤?s¡«Ò??`u÷-<†ì?`˜©¶"š?")·WD]q?pAáHÈ,g?ï±ß´íX?gœÖ8QY?bZIðŠ|?K²'Æ5å?~xxiJ«?d謁9~<AGN4FGL J0906.7+4950?èíToÿþd@Dõn?x»ÔÀ;•X'ßBÀ<ÚpΟ4ä@JÏß%ë@RÈqz?Ì\K‹*¿Kñßő´?ÐØV"¡jž@*6jX‹?ïýùà¬'¼?ÈÅq¤2#ê¿ìâ?z¿¿®UÙa–Ú¿é×»]Ž¦v¿ïåj‰
ÖAGNfsrq87GB 090322.8+500444?ïλš'?SÿÄag{?lä´Ñ'­H?Œÿ¿F#Ú?eµEkÍ?b¸vÖÚm?ïãyØÅ9Â?l?Vû¹ó?;/¼LÞã?F¾Uàb#?i Cw½˜?h†úÚv"?îê]Ãnn?"lIAvô§?xlxS?€ø¼wé"?œ¯Bù#íÆ?ïÅdžq?ïæ¡@›ÀT?Nк˜K©g?Pm;ʊíú?;V;T€nÝ?a(!?Áe(?IP"R%#X?ï»Ü%@'~?B¿Xʐ?d%‡Ã•+?mý÷TDVÅ?xÚ¡TV¢?x¾0˜÷LÆ?ïfŒ·?"øÅwc¦Ó?P¹aþ%I?\ÆÐÔå9?†¢zÊÍ?ƒM[ ?î,®1´¶‰?šފ~7'?'¥úxö¸?†©ÆMÜË«?¨‹žG<û??—oq *w5?ï±÷z[¡ø?mþg³Õ?ió÷эÇÃ?^{wŽç—ß?z
FÉ˸?gCþ	Ã;ÁAGN4FGL J0908.9+2311¿ïf©EšO2@Cô$_ZÙjÀ9ܺã–<îÀ<%˜°eù@ çW˜BV'?û
RH¢0A?¼Âs,lã?»óÈd2Z@M€ÿnàˆ@[,þåÑ?ïÀ¦]ø-Ï¿ãIJh!R¿áŒ…0aÈ¿Ôð¤ÃCa¿Î-)ÙÃ*b¿ãö9þ(kAGNbll3FGL J0909.0+2310RX J0908.9+2311?ïpÕ¼ÏB?'·ÅÞÙÛ?S±&X¥LÇ?Aezï<Ý?ª5ù*0¨?'í»wo¿?ï¶Ïb(i+?{—äfà?Tª#ÖzÔ?ZíËå]F?mÅø<¨*?w]—[	¿?ï)b†KÍÎ?Š$ꗤQ"?`½ÙÜT%-?ZSŸƒaI?˜»óûS·§?‰þ»Zª2¨?î#kˆ†™?'=ÚÅ͘é?y¸¿.À'?_'K	Lâ?ª—AdI6È?â©¥Lͅ?ï
¯ìõ¿¾?š2ŒÍ¶à/?d¹PÍY°è?VøìÊÊè?œØ?‰½4?™¾J$§¯P?ï7˜ðô?—Šôœ;ãÆ?kh5ü—¼ß?zé~Àñ"~?•ŸöÕßÅù?"
T—]´?î'¿Ip?œ£ÖîÀ'?ld`æÈ?jéôð'…?¬I¦"g?›ŸS5êÅ?êÆHì$xR? ]ºŽddâ?^GßÒ%?|SŽÂ'öZ?ÂÛ];*µ? 
XþÕаAGN4FGL J0909.1+0121¿í©.·ùV@>í/IŒ;À8SÓíçÐÀ;¥­'ž"•@Á˜€iò¸@ì´^@ý÷?žT©œéQµ?¹_¿p@
¿ó v@ð8æP?î‹#Ÿ—_ƒ¿ã¯Þø¿è>þ#†î¿å¼Ù¿úVs¿êìÔÿ÷«¿ïù0¾
í)AGNfsrq3FGL J0909.1+0121PKS 0906+01?ïڋøI}?dÁ-;¶â?c(!."Y@?Xó4Â3ԉ?bLÆ{?YtàúÆ£?ïËӛ¦—·?utâú€T?OÈóV™A,?V¶ÝOcƒö?v¼–bô?s-ož?ï&dm4XD?'º*à¼3?‡²ú¾¢''?‹(íæL?Ž³éôG\'?‰»sÝ=€?ïâ':h?Sš£øŸ»Ö?S"(SÛó?@*|ü̞­?cܲ&
ì?P^Jڙj?ïÁlÐýwÔ?rS"2fq?iSpq­no?a酪 gæ?rŸß,@'Ò?je§ažÏ?ï{—H¨6?Š–w(À
ƒ?aD>Æð?pHыš¯?ŒÉ{òèá?‡ÅÕÎuß?îÂöwJd?—ŽX?¹Ž?ŒÕlJÚXv?W ³Ñú?™6†¨9ë??"j'7S?ïœNØÞ±"?vR‰Æ¤?q»•;ÁÅ-?cgIÙq"ª?€Bh?qŠâq¤²ýAGN4FGL J0909.6+0159¿â·Š(kÅ@?\œÃŤÀ9DkHMwÀ;ëÛd?D¹@"ØБ(@ZÜ
²p?·` SÇþ?¿äq.@…@Õ"Ü£Ú@e骩}¿ë"ÎÁnŸÆ¿ÜQj€ÒMj¿ß;t€¿àW1	G|¿çDP'èË¿èx¼_eóAGNbll3FGL J0909.6+0157PKS 0907+022?ïÆR²)ˆ?jgÒúqÌ?XÖó=6-Å?QD±%u‡ ?v¾ʏ,o?eu(UɈ?ïGŒF¨c•?'•,FÇõ?| ¥V,-?'Î þ^?
®þ²Wi?†í녓‹	?ïc†í?ƒ{¦O¶ù?mOù¯ì³?qT'¦ý¯•?æöËw,õ?¤E3®µ¸?íOpåùÍ?‰	6("Ä"?™{p'Ÿ&?tN>rp¦¬?®QàÛ=!?"ò,0ICÍ?í7Py?Öé·c`ý?qj›¾Ý¬á?nr"Ûû?†6ËÝÓI?|49TÕS?î	[²>'H?«Ë¶IÄk?'ñ_Â÷û"?™^xëpž?¦q"øã¶?¢1~¦n×3?î¤åڍÞ?˜^š¦E4Ï?€n€<Ü?€MØrÖD?¡–²‹¿"?"F¸r¹
A?é•àYœ~{?¥u‹nôÚ?­Þb]g?÷Vå3?Â0æݨx?¡}àŽgæAGN4FGL J0909.7-0230?îŠåæh@<þrÚ/­À8'æ:\aÀ;ƽÀÀO@#êç¿í@@Ñå:Ü?£+w'(ãÏ?¹ºÙ…AóÀ@mmÁ¤{@K¸»÷¿ÁæƒA¾fX¿ÞOX,翗¿äÆÄ	¯¬+¿ãò<'Î{¿ëùÍNY¿Ù#''%ÎAGNfsrq3FGL J0909.8-0229PKS 0907-023?ï¾<´ÿ?',éjªR?a"C̃é?\ŲWÒ¹?x RZ?€ŠÜ&ƒæ?Éî˜?†¤AS³?e·ûBw½?r°#–Ù…ù?"¤Î¨…tè?'?3à?åÛ?îe¬G?Ÿ19Æ?Ž{uð†¶?×?-Jo?¢'ÐCò?›/>-†M?ïÁŸ‰¿ÿ+?ZŠ'pՈ?f¶a\ۈ?KkSDè4?sÕ
s¢jH?R¶1,VJé?ïu2'€³«?-n` uB?e3"…r@?\'î@ñ%?f'4õ3?‹Ž¾"è¿N?îäðþìjÞ?¢zdIPŒþ?xkOt&k?…O6Û§Ø?G@ñ…ë?Ÿu·îí~¶?í§'Í>?¦äeÜ?'dZ"e=?'k¿|éEå?¬ÔÜ3Ç|?¤)îG
3.?ïi i[R%?x8œQ¶¾?{»ÕUk?f§]NÕ'?ˆ^?qÐFöì]AGN4FGL J0909.7+3104?ìU¯kN5@DõË£!hÀ;PKúˆÈÀ<ÎañŒŸ¶@ 7‡bàJ?ýñk—þŽç?Ë£ƒè­S
?·ÑêK¸»?ì[›Â=Ҟ?ýž…´Š`Â?åÇà~ÛRL¿Ñ›Dß­úû?ÊÛÿ…0Öâ¿àxzЀ¶t¿é6añŒŸ¶?Ä]Ý@bp¸AGNbllB2 0906+31?ïÅø+í'
?qj¯Šíef?P[Žƒ@Î(?EQ-Z?óç?xíH"A?oÕû÷<?ï"˜S& ?"Ÿ®wjo?gÉYãé¤j?j~{8	 °?‰`¶è?€‹÷¢?ïb¸Epx?A"œN‹?l—-l–t€?o[xáèÈ?©›h?z'^:1¤õ?îþo€&½?wN–½þr?~‹ôL9×?dâì¹D6h?˜êÙÌ;?r(ãÖ)
?ïxº°"[‰?òÀ…ûYä?bvÜ"Ý%?T'§²Z‰z?3œÍq0œ?€×$êp Ï?î½W¸3ôµ?Aa*YžA?w`ÝÉÃ÷?{^k!4xÆ?¡>hݙ`ª?š"…¢'?îÖQ ëN?Œ¸\H€V?wáÑÛÆ5?vag.{~'?Ÿ=gpzÝ?ˆù;O=S=?ír10'1|?"À(¦F¹?;Üåeù?gŠäN?°Ç-®b?'Oi´IBAGN4FGL J0910.6+3329¿ëËÕEí(@E;\B 6À8܈'=À;ØÆï=:@¨Xx4?þn­È$Ç`?ªˆ͝‹?§yê&Ï͈@ì6Kìh@,ñê­Ø?ïõ@YŠ?Œ²QUø¿áS£ìó¿Ù
µà¢Á¿âêÑÀ&¡*¿Üj5"_õAGNbll3FGL J0910.5+3329Ton 1015?ïɞP|^?o àƒb?K+Ôß?A¤8ƒ–q»?wÍR~17?ltC1ü>?ït~.P—¿?‹äöuxä)?pÅ~¦ƒtÛ?x'Ûhýã?Š}µ("¡?ƒ¨!'cÿ¶?ïR¸[ü€?‹w	n547?ià þ`˜D?sÙ£ŠŠ8M?'là[¨zç?‰ðVƒ‰%È?í±/Êì?ˆwˆÝ¹Q?šQ·«óüK?xAͤ"ë«?§Ä'†³Œ*?'㪂G´õ?ï]-X?~ÿ[Ò#!è?_£°ÒMó±?T,H¾KÞÝ?ˆéþô­¶?|9ýC	"?îmÚÊ¢ŒC?¢ë¢˜Y?ƒT€<}Ã?ŠJL[K Õ?¤`>5ôd? '-÷W?ï$fÕ?'iœ%æ?sœ	"7ۂ?y©Râä…ã?š8¹Ý$x?í#å£@?ê³úÚbrÍ?¢o1W(¿?®ŒQ¬M?'NPZéä?»\FQô?›í…àòL"AGN4FGL J0910.6+2247¿åWj"¥Ž@D;`(^ÄÀ:È­ƒ[jÀ<£_ëøâ@Fá'+¼@Œ—£TY?·à…;h¶Î?ÅlÉKR@/–@HÅl@ÜD!×?ÁâIá n¿Ñõª§&¿ãTגùlh¿ã·#240¿î0(QWáh¿ï骝i2AGNfsrq3FGL J0910.9+2248TXS 0907+230?ïÆ´®Ã?iÌSh"wP?iàõHK?`?žvY?æ?pmµtEi?`{7òsD,?ïÛeBqa?sÓ·Ò¸Z?FeïÚ:Ԑ?UÇàî.ª?oGܓÜ?q­S/[ô?ï·Ÿ>I?'•€wõ?ú¨–üJ-?ŠÆ.±	W?·ÉNuÖ?"2µ*
A?ïіôß̕?U=øu}s´?LVnP/J?2Ž³`Z ?s©·Øù½?S
<»•ì?ïŸ^{F®v?uÙÓ»gk?x¼|…Õ?m«"Q[ìS?x?È«×?i&ê* Ôþ?ï+Ãc}º?'éë/©à?T¾ßñç]?azîùgsx?Š37RA?'#ÂjØF?îk-GXP›?™-Ú·N¾Ý?™}Æ7-ÿó?"èÎßA\?™á7ˆš?‹SŸÞXðš?ï…8|Pç?tU1œòtë?bÖçÊSq©?P§ø
Ìå\?‰ü&ùáO]?r Å-ÙC‰AGN4FGL J0910.8+3859?À¡H(ÂR@EáŸÂ¨‡À:Céœç+ôÀ<‰>xá"-@1o¦Öîå?þ#êÛ«Œá?½R'KÕÁ?º<kÁ:d?ÿ	9d¥œ@
PÌG@Ü>?ïµ{™>¿à6]õ~œ¾¿ázd ¯…¿Ó>.#~à0¿æegʵ¿åšQ_™¿AGNbll3FGL J0910.7+3858FBQS J091052.0+390202?ïõí´g¿ò?dàmš:?'=2 ?#¬&¨þ?Q<ñ?KY?d"«'ór?ïÙOÎ/´Š?q˜HŠR?G•áüK?P #ý-cK?ptf# ?mœlrÈ?ïщPºò?fÅÔñÁ?Qï²üQTÈ?T‰`ý ô?xÂNÿ
´?bÅÙ#Ù_>?ﺺjìÕM?VæÐþ"o?b‡Ú0`æ?@å6v07·?y^ݏ¡uì?TLوV* ?ïóymî߶?BÂÚ˜}?3¬ƒ´m%ž?""a¿Ñ?T"1L!?@MMHÿä¥?ïŒ÷®¼…F?‡rtü
»?YŽ˜éà?b²º ӂD?‰A9ê–?"¢IÜæ÷ü?ï¢Ç÷¿®?s&ƒí¿Ç?ZSµ;cò?T¶Ù%Œ¶?"0—jð0?q9g5‰q?ïCœí™°?s¨#o¥»?xÐbJÑI?^ZMY"
?'†nG·?qvpó{ÃáAGN4FGL J0911.0-5047?¯'L²¿üð¾'dÀ9v,:ñm–À:åÉêpL@F\…¼íÝ@Œã›EkD?ÃÄxÖ*š?¥
$:qì?æìË:%•¼@s]Å­õ?îoÚê¿äÍ]"̃¿êL!@Âgï¿æ÷ ÈÍcÌ¿ÞMŸ½~ü¿ïÿâ¾÷!AGNbcu2FGL J0910.4-5050AT20G J091058-504807?íÈÍÃ[£¯?«+µèê±?iJ¶XÖS´?i}ŽáÎÄ?°ï<2Õ"-?ª©9¹xöÑ?äi]«p ?Ë7¤ßop?{¨¿U;+?‰HpšA?׌ŠHTã?Ê©-éÐÇ6?åÅó#ù"f?´Yѳø{¸?'¯»Q̽?'j/ãaRš?Ò¡ž¼ªQ?³xkø¾ÆŽ?ê¼1
RÙ?g¬¾Q?jµîËw?Po(55?ĤdxöP?*}?|¸?ìBW"y?µÿ`Áˆ?lŽ:€ù3?iB4êT?¾Y{u°õð?µ¢¸Eù?ܩȌ‡s?Ê&f5+?uÏÝbn!­?†——"]ç?á{ÿ2ƒ>?ÉÞmôz:Ú?å$Åcç?²éR¤[¢:?›ÞA ²?'®àñ´ó?ÓúúÁˆ?²P<ì£	?ã²|êa]?±b¸~Y?'o·àŽñ?n­³˜ýt+?ÙKÿˆòé}?°ùR¦ÓÚVMIXED4FGL J0911.7+3349¿ã…x;"Åc@E_0"'À:}7褚À<FÞ˜¯@1{™>@…¼‡Û+4?¿Žù£?ˆ™õ'œWî?ˏà³3ž"@Gò[§›?ÅïšØL¿é,*?ï"2¿ã®"&±¿ãhpa'ëO¿áRG•ÀÇ¿è‹Å .AGNbll3FGL J0911.8+3351MG2 J091151+3349?ﯣL(€/?s˜oïBk?\†#
«?N"Ùʬ5?€†YN¼'Ó?p—Y¶;?ï£û§x ð?}u³Ÿk?Ve7d+y?U-ÞR5ÍÜ?"4o8ìƒ?{þ©ˆ`÷f?ïhÊ?ô?yÓ¶
×"Î?cµ#0$l?Zµ:ÅZàõ?p'3¿ƒ?wÜNŽp?îæ"Ùɵk?t>zWE¸?ràH孏?Qº®;åý×?žƒ'Ár?se
ˆ?ï+çH4]?ˆS	í]ž¾?qýôÛ\N4?aÇ«X†?–%ãfÂ?†¹Ù1"?ï0`<x#?"™ù-+pí?cåJ—p?gñÆ1ú7b?šÝCË-{¾?'ª×ӒÃú?îœ05/•M?'¤n¾Ph?rÔ
éõ?g}.ûè…?£â{)²;?«Ö$gÒó?ì"*vB?'ºR¶Vã?Œ§Ö­¨¬?rþlý]q?¸Gؓcü?"7=ä$äAGN4FGL J0912.2+4127¿ÕÇö…5ù@E«ž¾œˆaÀ9ÍÆÇÐÀ<cJw—@¼³äsˆ@\±×?®žsóí£?¦-4@¤_ñ?ñäB"ßÎ1@€"[ï¿ì¿ÚÆÁ—"\¿âµŸSí½Þ¿èܦÿ³©æ¿ãµZTà,%¿â븮㮿ïÿAÿ~ÐÀAGNfsrq3FGL J0912.2+4126B3 0908+416B?ï÷HŸ@?BÐ`ü2?2œV<ÿQ?.ûǓªP?I'†4íßu?;Mpo¿?ïãyŠì"Î?p»hÚµœÈ?9Ͷ±b?D4}­AÈ?iL¾ÜÊ6?n߈xÎ_¬?ï´76?zKwD&˜?YØÿ,XŠ?eû1,$y?n=¬P-ÿ?w¿KÅ|Q¯?ïþ"ûá?Fb&©h?ðeªßá>ð´VW˜D?(@¡¾?dâځ@?ïó úˆ?JπI5ƒ??~µ7Ô	?8ÆP|ªxÅ?QàI:`?DD«=l¨†?ï—p‡¸­?•rWÜ?Irléä^'?V½Ã®	Ïø?ˆ¥ýâA?"Ê•(àbÆ?ï"ú­¨Í?€ÎPÒͺ?buƒ{ÔC…?f˜Š_Ü?Š#ó¹ÆkÒ?}w;*o,?ïúÆD>ë›?4ŒÐŽo?!ׁ"g?Hºó¿ä†?@q
èì9Ì?2£Œ.AGN4FGL J0912.2-2751¿íÝ:in"Ä@+×ß°Õ À:w©"ÉÀ<´9Xb@(½Ã@Ë—¦zS?ź†c±Ö&?ÓZ]-W§@
"Á{_ò¯?ýæϧóyŠ¿£ÝëœàdÉ¿Ý»÷<Œù"¿è_}¾ò™¿êL'ÅA¾¿æʳ¸(ÐÚ¿ïüƒ]œ"AGNbcu3FGL J0912.6-2757PMN J0912-2752?ìsÖØOž	?°ê*f9?žǺö'è?"«Íž?´ß×M
·¿?¬h…UçT?äˆJç¯Ò?ʃûÞÄWD?Ê݋Ù4?ÃûEˆ M?ÂíFbK5?À*¶à¯á7?萆þao\?­ç©îŒ¡J?³ý¹_aÙG? 'j/¥ˆ?ÿV$h¯?¨¨Ž'ï$g?ålW/wøñ?¥Ù¶Eã?Çز*¬s]?¢­‡àz!Ü?Âuñ™j[?¡-üù¡}O?è/ cš%¨?½{#Rü?±.äÀk?¤æà_í?Ƭ3¦0è?¸ 0\ 1?×|}©ùä?Ìü
>¿¥¿?ÚTóÞoÈ¡?͆x0#šu?Ì]ï,¦°?ÃòCÁm?–?äê+'dÊ?²ËŠ øö†?Ákf•á(N?©Á^Y§')?Îð¼D‹?°(¤üñ?ÓZ4QÉÔÓ?ª"×ïóx?ڀuÆ« '?¶™ÚèÇ¿?Ò%U犊ª?³PÅ\™r¨MIXED4FGL J0912.2+2800¿ë0ƒïŸpÚ@Dìä¸{ÜðÀ;REå"TÀ<¸é_ªŠƒ@!þfUõU¿µt'ÞÛ?æ$ãåF?ïÿÿÊPË@Dʄóð'@Ô«-•º¿ïýH_ë""?ïÿå"m/®¿ébP¢Yܕ¿álpk¢æ?âKYÎy¿åÍ+Í
dmAGNbll3FGL J0912.4+2800RX J0912.2+2759?í´öȯíÕ?À$ùźp?›Ñ'?žt¡?²¿ÒûPrþ?¦ÇÊØ¡"Y?¸"%°o%?ï"ÿÝà	Y?™Z/ÛÁ°…?aaó!¹¦?tulÞ6–ê?†x0»=&?•ùà?ì
G?ì<ZtsM?©LÜÄ¿÷¢?£ïÜ•ûQ?œc>öc^?´%enö?¥¿OõVpß?î5q@ßï?ŸhøÌ`êq?1ÇIAõ¾=?7\cLùè?¬…]c½§†?Ÿaâ'""?î;»ìÄ}¸?²òÄàȖØ?žËIf'µ?¦o¹á¸—6?š"·âM]?ªm:xÉV?îéIUgF?ª—I-&›ú?sT¦ýݟY?Qÿ6ã^?ž«Žª |?¥ãÖ<'ÕA?롅[ýŠb?ªb¤|å? äswÇ?–Ýø"¼ß?ºèã ÿ²†?©.QãQ½p?ìÏ/)?±Ø»r¦H{?)Ý*%q¨ò?AJMoWp‰?¹y˜èËP?±Øø3'Ö¦AGN4FGL J0912.5+1556?ï÷š«(@C#,¾¤ëÝÀ:™&dî—"À<uÄsa÷@!%³fm?ý§8ô=T?·—•á|Ý¿«¢%¯<4?ó$ہ›v@½íc›/ò?âúw_²íþ¿èSľ
'*¿Ó˜Í¡ˆü=¿ÝPô¤­¿èæló"
?àã"C÷¦•AGNbll3FGL J0912.7+1556RX J0912.5+1555?ïÊ݁Oö¸?s=Æçßè}?SMÈ¯?MÚ®§Ç†N?u½Íre€i?p¦Òì'X@?ï£-ÈÿÒw?•ž8Âñ?]`ðOÉ*?cZ¡µ¿Žz?ƒˆoÅF°è?|Gå¥s[?ï6R›È?‰ößÕDõ?tÁ%¤â?}ö'ÖÒk:?"ÌHä?†¥%Q?ï×dþ?|æÏXÀÓ?tvށž±Í?Zij¹>"?™`m~ÂÂ?{D®I2³?ïp9¦dZ?ˆÚοCÙ?lÎb|‹'¥?e°á€)XX?Œ½ýÕlÿ>?…Í<ÈÙY?ï(Ë·_9?—ETç4?kä"yîc?v"åÅë?˜ÞUòa-?"U¶Ó¬³ÿ?îYkêðàd?—µ³%Ž?'¬";d3I?…À\)C?¥¾ @û
v?"*†m@?ù?ìëï°ãž\?šJ;¯Ðà?Ž}bƒL?}5nª2Æ?´ÜÒθm?™uHjüAGN4FGL J0912.9-2102¿È;…|¬#	@2|!ïAÀ9.qÊG·OÀ;à{.t‡'@ @É1aÌÏ?ý‹ÞÅó"¸?­ÐÂ¥¬wm?ŽÈfƒ4C?ဦÿÝo@Ÿ°É6¿ÜÛ@­ð¿åŠÉ>$(¿Ùeåvø…¿Ü=Ì4!¿âø?Â7È¿¹U@Ï(AGNbll3FGL J0912.9-2104MRC 0910-208?ï·§mË=?vÇ%{_%æ?R‹@­E¦.?H—[½þ¬?Í\2fŸ¾?tc(QÙj®?ïÊ
ˆ>•?xŸyc3x?SÇ°‹…¨?^V†eÝ?võÌ
GÜ?sz5?ï>ÈYÂá^?‡6,N÷æª?q¦@.õõ?vSrÎ>À?"½d¶EÌ?ƒµ'ÎõH"?îÓÓSú~?}ÃNki?rU×0¬²?T—Énù#ï? x'Î@½?{£È1^?ï]‹ŠH?ˆqe"ô–?eâ«Ô­2}?Z¼ñY"[ð?''9>j<í?†XŽ•IÃ?ïl!šô&r?Á}Ì$*?cs™m²?qq'¾µ?
Yn?‹‡©1[$?îM¯`UUG?˜±:0c±<?›ñ¸ì|Š?€–Èž´Ên?§1‹Ç¬£ù?–7ȯ‹è9?í5»mÿ·Ü?—~+±Ü?"¶ÁðMõ?mêŸ?³»LR7d?•¡\z'AGN4FGL J0913.3+8133?âíç•Gr@?ʝ@îÙÀ;qøòŅÀ<öŽhãï(@!¿ì÷åK?÷ìˆÚ.µ?Íßa$FE?ÅgY«m´?ûB=ú	F@Sx]3â±?ìäâ½ÏÙÈ?ì6«Ô.Á¿ÚÙ=—À|¿Úͬ;ç%?µ‡Kä/¿ÒÀ>ÉêDAGNbll1RXS J091324.6+813318?ïÙ7ÞW}"?j}Öx$Ýc?Iv.¦Š?AÊ´X´{?p5M"å!î?gr…Ð,\c?ïÙ<a&­á?s‹½;?Bã½('Gx?QØÞ±ÜEŽ?qWÍ°CH?p<‹N
И?ï—'"0¹?'»°e{?WÒPIåkp?cOõœˆç?¯ö
/o4?û»Ê1l(?ïÁN:ºTê?bm‡"þˆÛ?H/Õ<?9M{E
:?|RÿêÕ?aåûUÎú?ï¨ëHZY4?}Ã÷•"·?\"ûv¸«ô?Rwk% Β?'2®q£¡|?{\Ýjm Ü?8=à?† ôt	%é?P~k1?ZðÐbJÑ?ˆ¤K›§?""€E[é?î:b¸˜ª?˜òü~¹?b5ø¢  f?jmB‹g?«6të–9Þ?—ÁJ¯óðu?ï=mŸaQ?ƒz
×ð?Y½ÁCèR?S«°'?–¶–II?ƒ;˜?N	þAGN4FGL J0914.1-0202?êÃD''@>-inX£/À:è½±¦×À<[íâÇ
@Á_»ýF½@ûÜA´Ö6?Ã&¥]Œù¿§I#4{S?ä!7Ì¿a?þØ^€¾×A?ïù%P¡F¿ÙsûD¯\y¿ç™$(Ô4 ¿èyÚçÜs¿¤L߁°CÕ¿ïlìýļ]AGNbcu1RXS J091407.9-015949?î¹xW]<¥? NÆ3@ú:?jÒ_&ŒÌÏ?fŠn÷:?¢»T˜GYè?ŸVþ|¬«?̠_º?ŠCöš"¤?h"c¾Q›?m`7׉<?‰Õ3ÜMÌ?…Ž†TÍ´?îØ-½Kr?Ž³<FÆýš?w.¼þ?tYl¼C?Ÿ.ØåǶ?Œ¿L±‰zh?ïAÂJÆUm?u«[Ž /?d5SÒm©.?Rít.õd²?•A13 5?tµ:¯1í?íßQ¬"¼?¨4ÀôÔ?zð¼pR0?q0ý‡Uxp?®¿¬ÉdG?§_rä"¡?îÖF¹€r_? ìÅ)"!§?uÔ¦êsÔt?"UÕ!j•î?ŸÁÿP.?œƒŽŽza?í¸ôÓ–5?šæ¿s:8?'þÚ•B?y mSB?¯°üKee'?˜'BXø¼*?ísAWR2?—x¥ñ%M–?$´LpĀ?wœ&ÖrVÎ?²A^¼ÞI?–x½ÚAGN4FGL J0914.4+0249¿Þ4¼šÐ{X@@h&Üã›EÀ:æ*|«LJÀ<X˜џš@¦A¡µòÁ@Ìî?äž?Á!95«³x¿°ŸíË{?ðn"ü¡¦®@Ӈ[Ôg ?íòãâ"¿é.î•tpë¿êt»(_šš¿âMaa™Î¿×&IaÉ¿áÏïH²AGNfsrqPKS 0912+029?ï÷8?DcÓØ8u?_ ‰rŠ?SAÀ1cpW?ˆÝãAûš?€WúéæÁ?ï«,ùª¨?ÈjÊ°S?\µþ_-o?cš1ñ«e?žÛfáh?y¥©—'ÿ?ïb¤èa ?v© :5?ayÅÖpßñ?S­ëiÕ?'|DÍyö?€°§$äZ?ïŸCƒ§.?dŽžÁ/5|?Q«¡GV?:Ç¨z3'?†Ï|xY?c"¶mmÌK?ï±Ý:á±?'/̜tl?pÇq-Ñâ?hç@Hsüò?š8ºtŒm?æà&úHd?ïK]~‹KM?`k+›Yû?bžYWÄ;ö?l<tpä*?"@…×Ù?Ž:ÊÉj×4?ÿ¤Í?'ûÙ£?qa=ç%t?n‹5'Šµ®?£;hU¼»?›'¯§?î'ÓbÏ>R?…ɱZ³?qFMÀî^?a~[y‰=?¤ºö'?"†Qµ¡¯_AGN4FGL J0914.8+5846?ï¿RÆŒA@D§t¼j~úÀ;U^½ûx²À<ö›]¾÷ø@b#¨§?úåP׈èq?ÒÜù€4à?ÑÃa~ ?ÿҖÀ¡E`@':g?ï¢w÷ˆ¿Ø÷£ei}¿á"i·S¾Ä¿Úa'¼]hç¿ÞÁ[)œ\¿ïÿíöé	AGNbll3FGL J0915.0+5844SDSS J091451.54+584438.1?ïÕȲÇú?gxyú?RVÓi-[?Fô
m!G?p…ñĚxŽ?cÆòÝø')?ïµ&Ûê™?viikJœ?Uh¯t×Ø?WB«f+?€›îÁ'Õ?rl¦S‰½u?ïSy¡ö
?ƒŸ轡?m'³ô~4–?jù{TÕ²^?'Þ‰!´??'Bi@'?©?ït½ñVˆ½?iÝöOY?pLÃn©|Î?RÇ£S¿ã5?Šª!ö ¸o?f:™'›ˆ?ï²Óa'jv?uŽ®Óm-?a÷árÉÐ?T/2"lQ?}š^"CÌ+?rÁ`´ªÿä?ï&
@íG?'ýUQÍ?j§°$IÝ+?sžâí—:ù?—éaáz'?ˆÿ€nÉ?îßõpQn)?‹é€Šõ?v16ÏCï?x%ë™u?žujÇè?ˆÒ‹»{ì?îŸXɕ,?"5ÌqÞk½?}_ÖÞØ?Ø?m©¯©Õõ?¢^"³˜F?'lÉ-»7AGN4FGL J0915.4-3027?î›é¾êG@)g¢xåÅÀ9ÿϾï"xÀ<49O¬æ}@
¾ýVW{@º–ic?¿Èûà3÷?ÄŸ€
s@Ûc[+J@ª¾MØü¿à–/¢!M¿ÌqÇXÅʿ㚾È'Kž¿á™!¶3-¿çY$Hµ¿ïýü_Œ'…AGNbcuPMN J0915-3030?wkØ|?²©BDæ<t?tÃEJq6?¡%f£?…8?}¥N?§,ò"ê2?ï¬ÒXIdš?"ŸÂiZ?_(û<Gi?g"DÖý0?€æfýi:•?q`ä2?ïx ¡úÕã?Ô®j!Œ?hÞcRSœ?k"?‹À>ªýȂ?~ÿZkkëÚ?ï5Á¸#Á?iM*:q,?|ðÕcsë©?U^ýˆ-:?'"©bü?e}, ý?ïq(X'£!?'xíÆzIÞ?|¹ViîW?†ŸÙ"s~—?…¦
Zˆƒ?:õ7ºN?ï?Gú¦¶?š¢‹:E??vTfy*É?+5þ‰œB?™'ýX­V•?–ÏY_àî?î÷¥å¥?'ï*""Ï?xO›hbªC?u™b©Ö­?š÷\~—Eè?ë}…õtw?î,§9&?…UÒðRbù?'ÆÑcŸ¢?r"ï̐@Ç?¦º¤'W?ã'Ý%+AGN4FGL J0915.9+2933¿ÓxõŠ0E@Ey…H©¼ýÀ8¥	pÂ
À;-M@$³@áòNço?üN™´?¥à¿Ôu?´FƒÇö#]@#¿µ'@	kèhߒw¿Û·‰lü¿×üè]÷×è¿ÚnYåN£Ò¿Ù‡'›x–ë¿âcÆ®¥šY¿á—ÙÛ©¢AGNbll3FGL J0915.8+2933Ton 0396?ïÇ¡fŽ÷¢?vLƒ'œu?M•|`â~?F¼W²Ù'?x|'u<Q?t¤Ã­å&?ïu»™°?'C`‡<:?oŽ)AO?vaPùQðû?ŠØ8Iî@?‰"€$J§?ï—xf1üì?‡×_Œ}]k?fQ@/Jg?vKœƒDø?"–eŽxt?ƒC Žä]…?íÏðÞyóa?3AæÅÀ?ˆjw¢`Ù?d\K©xi0?¬æT/ȓ¯?Œ%‹ï{½*?ïcL~ïÛV?'
os8-"?`ÔÖüd‹¹?]ƒC¬&2õ?'{ÕF?•Ç?e¸I:º?î]2"®§?²µ‡ìÜ?‰ABçòrB?–Å9j
Þ÷?¨yÜ|ö?®m/⩁?w")?–".wl'?xãÔæÍ°?D@?—"÷:«ïÕ?"¥côºÝ?ë¹Ú¢º?¤0‰½\,?"¿­^ÛH4?{r#ÉáÈv?½с$?¤_¥å©ÓÔAGN4FGL J0916.7+3856¿rõqSÐÈ@FؤTÞÀ9ÇÑq6À<Z«m×sð@}Š6OGf@ ôQvY?¶<Œß].k?»éß,Já¦@#³é¦ø'@ş\§ê?ïøª*s¿áŠ2¾™-c¿åV«¾	e"¿çøä¸{Üð¿èÛނ׶5¿Þú@MxAGNfsrq3FGL J0916.3+38574C +38.28?ïáû†"Ð?b#ÑYŠ?DwsçqÖi?8^ˆ5©Ò?hæœg6ho?`‡ÇK3?ïÖ±dç`L?qO!€wA}?Gíaý¢+'?SzxÛ͵?q©¡N™Á?k"ò$$‡?ïªfH¼åØ?umƒöË?a\ʾM*È?gÙ2ÏÄÊ?;*";]?q¨,È͜?ïÑ*Ûd¯?S§–G'³?d$P—?E–öPif?jÔU«ãa?Lë¹ï5U?ï´:Þ^€Ð?tÃp¢_Â?\UŒÜVA?Q§©%Ítà?~Í-£Yê`?ráo˜ª‹x?ït°õˆÃ?~îý·ú?_Êb}É?eìgúW©?ŽÚv|µ½z?ŠÖùíˆ}?ï\žƒ…¨m?†¶GIˆŒ?pç°YuÑa?r/ÇIÔU?2C~lÝó?'tåç§?ïm²‡1?tA¾yIJ?€(ÖÒ£ë?fÑÃÕè?"j¥I×ã¢?nP•bµÿAAGN4FGL J0916.7+5238?¢Ýy¢–3@EƒÖ¶Zš€À;96À<éaB:73@ ©³"Q]ì?ûbU)þK?ÈvnfÔ?Àž«;ØsI?ùŠý¤/ö@›‰¿ÜÏN¿â±/bn4;?ï[$éÄT?¶œ µÍ¢¿ÝåœFó¿Ú/¼TS¿è®ÏÁsÓ6AGNbllRX J0916.8+5238?ïà§Å"Ö¼?\½¯³?g´?@éõ(÷§í?4ïSŠ6âz?k½×ÌÓ?Ye#ÿç;ñ?ïÓââ|¦3?tKÙ^ñ¹?Jaž²Å
¯?SïO¾?rÂZÓj0¯?p­©öŽ?ï…K{ÔaÂ?r€f5tÇ?^CŒñÈ?\ÍCU£ù?Šä¯zS±?p(om@‹?ïr¡¡êÅ?j¤²N^ÄD?q<ýãIJ?V<͕Ü?Š¹ýâJa?f/Ž¯ž?ï¼u¯.¬?mÎõ+€?WKBYzõ\?Lè¹ð<RM?|&ô°F|b?iUû[iÖÞ?ïoÌ¢õ&Í?›\Âl¯?]
Ír`	?cÅB¹;â?5ŽÏˆ‹L?Œt5;Òè?ïh¢›?ƒáÄO؉ß?d¾¯‡ß?SI>¶<É$?™»(#ypž?'Ý£S?î»
K†Õá?ƒ×óK°S?}Âx'\yù?lFø–X? –ÜC*?Q®hq¥'AGN4FGL J0917.1-2131?èoè+‰+ô@2ëÊÙ­…àÀ:¿ÒóW{À<WMÒ@ê{áLá…@ÊA¤åþ?Àoºx¿ºc%¿,P@?üuuGª¹}@@Ÿ¼}¿ï»…|¬#	?ëÈóĈZ­¿åfl{S]u¿æ¼QքܿÕsϛY–¿á‹½m´8AGNfsrqPKS 0915-213?ï•ó-ú¹?7WôÍ`µ?X·ÎPO?[í­E§½?‡q=×g_ª?)ÖrzâC?ïԂņv@?~"sW¶®?P~pÑ'ë!?i?çU/?qŸ#÷Å	?tDEc¾>µ?î¿R‰Ë×k?"lf¤‡†?{ÍýNë?€Â
NòªK? '5‡vVs?'¥}[("g?ロè7È?c"{½Õ?Pq´lù?CD.'"s«?|–tZÑx?aJŽ&pn?ï$_?£L¸_ž?k)wÅÝ°?gVük>ö?˜ÖMÀWg~?¢÷ÇË{Öõ?ï}Ÿ~œ#s?'à–ìÆ??dŒC<+B?{
'Tš•O?‹u'œ*'?Œ3>ŒPÝr?í«Ö%C¹ò? 1)"_.J?"Fõßu?‹³à—¯ß?­úðà8¡?›æ׊–þ?ï0¿Ö͵3?…&€E«Gü?k…Ÿ*–ñ7?e"OÝ%?–wQAÒb'?ƒƒ=CзÚAGN4FGL J0917.3-0342¿ì»"n›Ë@=æ»frû À;.Ɗ"lYÀ<˜-שŸ¡@!ºÏ ;Ê1?ü»-Çüƒ?Æ˛ÊKh3¿•ò†Hõ?Ñ%'×µ^?ÿCûàa¿ïûjÚim'?îƒÓ"g*²¿×Êühñ¿â×ßð•ÿ±¿Î-›™¤{¿Ô￀ˆühAGNbll3FGL J0917.3-0344NVSS J091714-034315??ªÍ?kÊ-ü‹­þ?E´—=Ëö?5"n•BD?~ù—µÛšù?j25J9µ?ï­ØÊuÉJ?¯‡Ê¾??Tµ˜MHC?ZÊM`ñàj?óZôi0?_f÷?ïg`eôÉ?xés4Ÿ©?_#ré_2?Hñ•-R?'!̅3˜ú?x"coúƒ{?îÄ©s'…?'rpå9l?ijþ°Ýs‡?T"¼zb#c?¢¸Þˀ[?'¬Bæ?ïp&)p¢ç?Š‰"š?Xiç•r
?O,Œ¨ªæ–?z´+_7?‰<4«Ü¦Ú?ï À^R÷?™å­¬;«Ô?c<PM(\€?j€g[Åí?™€j:ß¹‰?˜Ú²þy|?îà'/'¿¶?‰U8Qç9œ?eÍöGaiÛ?ZJ"ü	|? š
¦¿n?ˆƒh9V68?ì[ö$×GG?ŸÓƳzŽ?}2šr|à?qqömª/m?»M-^¡º¿?ŸÅK–YݽAGN4FGL J0918.9-0625?æ|'­l4\@<©ÏF#ÐÀÀ;(ZµX<À<§ƒ]2L@ÅÐon¢Ë@Êô¯ú?ÏâXûå?Ó'{ˆŒ?ûûCµBm@ó^'í/Ä?ïã¯1±Rô¿Òþ"Õ½6W¿âòžM]€å¿èú'7¥ˆ»¿ÜõÿRÛð¿ã¢"Ÿg8ôAGNbcuPMN J0918-0628?ï€!k")œ?|vܾ"??e‹4•´ø?V'ñ†v™h?Š"×ç'Ùó?yÖº]õ®·?ïS$Õv?'2꺨ÅÍ?vpÌn½×?yiÖúv?þð»í~?ˆ¡{'ûþY?ï¼OÑú^?ˆ¬HÃÒÎ?|'[¶*è?wÓ=ºU½Ö?–cñmËG'?ƒ=êÙ¨™?ï6²x…?s
la?yŠÎÝ>¦+?_0yÔßA?'Ü5ô¤DR?qì"á(í?ï
r)y\?ŒÅè_ˆ"?tàyI¼eb?jS¹ÓÝJ'?™…³kya?‰¡-²V?îV½MAÁ?¥q#~·Ô?ŠüOoŸ3?"¸é0©Â¼?£ÕND>p?ž	Ÿ+¢ò¾?î8{NªÝå?—›Ä¤Ü¯?ŒÍ;!ï2?†4ÿùæY'?¥E	Zæ?'÷¸™ö
?í_ÒՋž?'xÅ$¤r?'ê͌çä¾?€úpUÉÒD?°Lnc"[?€4fæžBAGN4FGL J0919.3-2202?ïæpOt…@2ù€ä–íîÀ;rûbÓÀ<²'{J@!VhÏÍ2M?û‡"7Üæ?Ô"D¾Â?ÂÊ·H×	g?íds²C­@Á5±]†?ëޖxÓ¿ïynìFå˜?à»ÙÊâ¿å5ü;Oa¿Âák)¿é$ô^NAGNbcu3FGL J0919.5-22001RXS J091926.5-220052?ïÇl‹Íà?€A}1±¹X?DÚ-±Ï?O0$Àý9?y®tmøB}?}=8<(òŠ?ï!n,Xx'?ŸÐI"xÁ}?k1MW²%¥?q5|6ýÛ?˜lÍÂ;?žGEÔ­?ï#¿|†?…¼©»'[?dðΛA?ib¯<æÂ?™dï®Ì?"‰­9õÊ;?ïs—ý7N?}Œ4<ÛÆ?P8"6
°¿??pdì(.?œ®
àpÓ?}G,CUÀ?ïmy!ìu?'ÞՈ¿?XŠ½âH¿?Rüæ?ì?È;‰7ë?'CI ‰	?îTwâ Û?³Ù_XSw?uú÷®"ï?‡´­'Œ?¬[uZ"{?²åy|NÍF?î#÷´'?–¬‰?Â(R?l"™žxÛÇ?mf¸ÔBþ?«ýíWç¢?•ÿfo+?í?¢$W£*?3õàHS?Zö˜€ƒú?VÑöwT ?µ—{"}?œé¡ta-AGN4FGL J0920.3-0443¿àº…Côª@=ñ|^ö/À;+×õûÀ<W$ü8Ë#@˜"vm@wŸ©~+?Ë\(	‰k¤?´€ÊjÇÊ?äIRÄÈòM@	 ]Ötì?ïòãízÂ>¿èHyìU(Q¿èjd!舿ê1HKÿ¿á½¼>	P¿ïùœÙ¿úVAGNbcuTXS 0917-044?ïò¯ÖG?N9Sǹ?)ƒúm
?.Žý1?Wq›®Å?K°S6®Ê?ï§àcyïR?ƒGò`Úz?aKéÜ~ÐÓ?iŸ%pç¥?´ì«ÄO_?~®ßá°i?ï›&õÀ¿?s¤ùn X?XXfªv9,?Dö!~Ñ?†+5ºX¡?rÜÌJÎ?ïmÌaB?c'—{{?TÈ®½g³ÿ?9c–7[?†wR™°?c¦RW"?ïå0•ì]X?b×Óz^À?3®QzkD›?,¸Î‰áŽ?hYŸ½üΓ?a&»Ž?ï67Qt¢?™¢ÒMKU?h>ÖÇ¥Û?w]É´¿dÚ?–5®	S•ó?–*lß?ï7Ìú2ûD?"5Ò*ŸÝÌ?g@õq'R?cJ_Î]wÖ?–$x˜2µa?'‡×˜äX&?¬:—<?…1AåU‰?p÷ÄųÓ(?^à"ååÌr?£·œ xb?"r½2`/'AGN4FGL J0920.9+4441?ï*Åë 
Ö@Fgb(EÀ7ÉÑæèÀ;8àò¿@Ì8¢2ðB@#szK¹? Í&Ü/7È?Ár3y)6°@&…ô¡'-@®uµŽÂ¦¿œæAE£*ð¿Þ%[Z™ª¿å&=·³à¿æ°üÂ]޿ꨢ ÿ>¿íêi*fAGNfsrq3FGL J0920.9+4442S4 0917+44?ïnh`^?[lFÖýH?{'ªkß±0?(ÚX•\7?†´P¶-Þ?1è·7Yö?ïw­o©?—5/«¢]?nâ–~'J?€
Ì7£Ê¾?Š[þd'¨s?"RWã,9ä?íւæyÇ?¢ÐO«}¶?¢Å–'Ã?:?ú=8_?Ÿ¤v߈ÐÄ?˜rï?ïsӒAi4?ƒ§¯b×Ü8?lù€^³`?d"IvÖ?‹Ì»Qq¯?xm¯Bé®?î¦!ôÖ*?¡ñܝÎ}?"­Ÿ?øs?"ÖBâ묓?—Ž½Ý¦M?•ÝUz½2?îjØ/v»?ª¢=«Qêé?ƒl_M½(?"êeÀÍZÔ?¤wf«ëÈ?¦÷.A©:?í^‰4"ýÆ?§³$Æc9?¤î§>À?  	1me}?¥)X¢…/è?Ÿl‹?îDûà¿%£?Þ{Á‰¦?…ÿmÝë?}"íùÙ,?¦LBúS?šÂL¶ÔøFAGN4FGL J0920.9-2256?à(:­ê£;@2¥…7âÅ]À:ÙjÿR[À<€[wõÚã@!$ï$©Á?öâñLO?Ն¥ 5"?Ö¬ƒP?ÿýf¤S1?÷°o̖œ¿æx="ßEu¿àNÏÜKÅÑ¿ÎK*
j'¿»Õ9'ØŒô¿àš¥½ê0á¿àõ–AGNbll3FGL J0921.0-2258NVSS J092057-225721?ïDÿ0?¥¼ÆGâº?bŒÍ¼_?lA%ÿ3øc?MÇcL?¤LìO›Š?ïQc¹§›?—-­0{þ?|‹FbïrA?€",·þet?•sð¿?'P•³tÐÑ?îz'k~Ô?—îQuM?'º?ÿŽÞÝ?‹ÂØ•}?£®ùK\ª
?"â/@§"l?ì;ë‹~ν?'Æ(Ý?‰¨°[ÿ€?oø®ô:ø?ºë›ù4#?'¶ñǘ?{PƒP?œ¹îá'c?hiÜl÷?`ùtûž.?£Š‰Í/?› …€ŽÙî?í–ç4y{¹?¯û3w8
?"µ|ùû¯?¡è0¯P
?­±ùëF"?§7‹)å
?íQýš`x? Ùíã?…×Fs7øB?qÛ¤}æœ?²µ*c%Ë3?ŸÔ›MMæ"?çê໎ƒ]?¥t>®¿Û?']aÕ¿?"%I*ãN?Î4QdæMk?¤ég?Ý AGN4FGL J0921.6+6216?Ƽt^´k@Dᆘ5À8LPíX^À;ê"lXî¯@"ýð[GN@ÇìoíÏ?œMÜ#N[$?µFß•d¬@2è8ªk@¾j£Œâ|¿ÆÉ™;¥È¿áΪó^1¿ãÝ_~Ù¿å‹V	÷Ї¿èém¢ð¿ì,ÉVö†ÚAGNfsrq3FGL J0921.8+6215OK 630?ïÔY¿A§s?‰ñßvhÞ?W•O bÉÁ?P!(Î'ž¤?oۘÜI0d?‰Û͈3Ü?ïÅ]ÒĬ?~¥³àÅ
·?M|M¨»R?WÙvR¾{?y¡"ÓÑâ­?|Ýƽ'·ø?ï¿VÐ)E?Ú:@g'?`ujRÀªr?pÂðk2?xBUÍØ_?yepÿeá?ïý+Gèˆ%? ÛØ ðñß?¢uÚb?	ØFË6y²?0Ÿ–kŸñi?ÄóöuZ,?ï±0ñ	?}¸°\¿ùŸ?]"Ë£K?S~«&RÞ?€JÀ ¡ ?|ŽY@Ve÷?ïnš÷ßí]?Ë¨Íx #?[¶ä‹¸ãê?j/¯Ôo1ª?q2±ÓÙ#?Ž1'Â'2?ï—rÑ~l?…BÇ	p?y?i
€Y_ú?tكB­ã?ƒà
;Ù?Êðÿ_?ïøÕÈZ2?@áéS¶B?,RÄ>3­?#í?Âck?E".-¯šÁ?:º$ÆnNAGN4FGL J0921.7+2336¿ææŸçÖ,@ElÍJ¡À:<—FÙeÀ<xÀŽÐè»@¶õ¼/E¾@y@þÍÐÙ?»Ø5õ…S?`¢1Áä©r@K®+÷Տ¿ã­ÕÀ­¿æÝݖH¬A¿àîŸéiæ¿Ú$;ɄĿéÔÞF-⿸«äIìPAGNbll2FGL J0921.9+2335NVSS J092145+233548?ïäZCÝ[?\'Xæ¡a?NÊ÷Ÿ©_J?AxÀMÿ?còþ9F=?V¬ž+i-H?ïÕXÂ8õ?rÌ!z§ÒŸ?I"ôôó?S"*£þX?r0dHÉ,?nÒº1Ür?ïƒ
~o?"ªÜ)/P?[³ÿL'á?b¨¾xžy?‹Å¹"(
?"7K>ï^?ïÆȃ^f4?Wa€Íŋ?U>º9õ¹?8ž¤ß£ý"?wLÇ1?T´ï*ƒ­è?ﹲƼ<‡?u­Åàq\Ë?e6lóþ$î?\‹¡ÈŠóa?x‹f.ö?qbw2UW?ï…Ü» ¹?o=Fÿ».?ROú>Î?_á^Ɓ©?Œ>þ›æuÌ?Z·ûg;?ï<KRˆ?1"ïã1¦?esÆr‹Ú?f·èÚ·€'?™©ýÖ4H•?ŽÂ‹-Ú©?ï]|`+ls?xÄ*Dô?l£>Í?WãÕ¨—§?ÌŽÅD?vIÍÁÐؓAGN4FGL J0922.4-0528?Þ%iÏ°
@=푼U†DÀ9õ×CHT-À<WBXj$a@í™IÁÉ@[A9†3‹?º½ó×þ"?Áû¿i!@¿l\I¬ò@I1!`"?ïú=³¿µ?±'Ò*.Ò¦¿á7€—9î¿äW~Áüå¿Þ:Ó²¿êc'@ßÄ AGNfsrq3FGL J0922.4-0529TXS 0919-052?ï©ïD=i?têÑ®'­?lã"MŽæ?l&9i•\?|–"&t%D?j`m¥ã;?ï‰Ãl'?†[ë3ßC?o¦&€Tqš?tTLt?…Õƒâ"?|²Ä-®ôQ?ï=Ão€ìO?†<)vi?ti\ææù|?uêƒPˆ×Ë?"-:ÙlXÉ?'`ԀÉ1Ã?î[ 9=ZÌ?}f@¢™´Ó?–ֶȍÿ±?t2`'Îa•?µB
Ÿ<Ý?sRojÇK:?ï)k%_Wv?ŒJ"­·?ˆÆ3÷…?'' ÝÿÒÄ?pt3
?‡ïhO??î·$:X&Ä?Ÿ|ñÞ£:·?"ojÈ«?ŽW®Cž&?žãÃR]lƒ?•²Ý™jù?î"P®²õ$?™°^€^¢1?Žº˜p8r?Š7‡µÿFk?¦,NûVF4?"²kú.lÀ?ëÙ8³•T?•­½¿ø?«Ëzز_î?ÀÛD3\?³P'Žxä?ôÁルBAGN4FGL J0922.6+4454?ëDG¤üœ@F‹«ud0+À9»ˆpSOÀ;;èné§@lY­ñ?s@µyyh¡ª?µºÎaf;7¿·B~"%¥@¨š¾\ǁ@zxnљæ¿âEà_PÈ¿ëÕ®Þ]¿æ4ò»sÞõ¿ã'
?ىʿïò5ýgõ2?îÈïÈzWµAGNbcuNVSS J092235+445749?ïñèïÔ?`kG
;?;Bƒ¤Ý49?;àºO–†?W#;·r?\ÔÚÈn?ï™x½?Œ7¬?fè²P0¯I?xó9?ƒç¢²»2T?…`(CFúÜ?îk…˜ ?žê"x"¨?ˆ+$Œupz?ŠŸ~ǐ¡?©…ñ}í?›£.Ú¯?îØu¬¡Öv?‹¯ø^T?bÈÀÕÈöá?T,«ªÌE‹?¡L$'|1?‰ê¼#Ì÷?ïÖ'"[«¼?wx•¬fÞ+?[=hœpÁ?`î›ÏöS?lXMàçÕ?s¿‡¶‹vz?îðöUdéí?¤¡àæºR¯?yEÎôuÚa?—õعÞì1?›Ášݾ?îه³?ì»W_'?§«¾ßI2@?˜ãÎÑm?"ÄÁü¿M?´ ŽÜJoð?¤÷­IowÂ?ëÕJµ¹hu?¬=ã¾Àju?… UI?}[¶•"?¾±§Ç¥?«KOՀPAGN4FGL J0922.6+0434?±~_Må³@A»´_½ŒÀ9Òþ?5 À<7•óëï@šÙlmf‹@͉ößÆ?°&Ëƽi-? 	ߧÅ×:?ëG©Â†¢Ç@=zœ©C†¿ 'Ѐ>T¿ßz}	@¢¿ç.,Ε#é¿èëaŠR¿ç»š?±Æ·¿ÖŽƒ»áÂþAGNbcu2FGL J0922.7+0435GB6 J0922+0433?ïø>ŽøÎ?<©|?r
?&š:_Ó.?ub
ˆs^?I_sŒéÈ?9÷mVv"!?ïæYéUnœ?hÛ@Ïô4ž?8ÚëÈìs?D\˜0¥ž?fŠ¸ð"Úš?eh'Ž_?ï³·ê~?sš eGÐÍ?ZPÍÃ,èÿ?`âL£¸$¡?×§²é!?püì8›§?ïù†ì:GÇ?*ÓUК0?& ÏMÀ?‹ŽÒM?D<HŸ©é?(-{w)Ñ?ïòË;I¤†?M–'§är$?/`+Vâ?Vè¨?V}…2¢ž4?L‡ýWó-?ï¬ÿ¦Z?"9$Úê?GÔÖàl†­?U¡ü	Gr?ƒBì"ÐQù?'îZäA¦p?ï_dÆE…?ƒY_ù?iPá9)?k¤+ü[Ó?ïÒcÏ-0?oüØOWA?ïí,J®~?Oõ#ª—–?AÜoÍ?,ÀÇÒ-\?]#|Ç$æð?L	ãUšìAGN4FGL J0922.7-3959?¾>˜×|Ô@ƋýϤÀ9sÒì¡~jÀ;ݸçì
@}"£˜öÜ@ƒˆ›D"…?¶hÛ¡%ÿï?¾¿Ïä.hH@Aƒùdo@Eìs±(¿Øæ4"E¿æWãa
áë¿éZ~›çQ³¿ã'ÞÑ·¿ì
ÓØZ¿ïÿƒmÞ)ìAGNfsrq3FGL J0922.8-3959PKS 0920-39?ïÌ@&´†?i VэƼ?VÁlŽü?QŒ6÷¼NJ?t/›RD."?e«r}T£H?ïÄjÚr?'ö2ù[ß?BŸkšt·??S½u´¦6?‡e²)Z?'üŠùšk?ïKý~'Ïr?…i(˜¯?uyébžÍ?wõ]'A¯<?'!ì2?€¬–l*°	?ïêқ1¸ù?DćŒÿ‹?;+ÆuÏ?"
€FŽf)?aÈ&ì¶÷?C+D(ˬÿ?ï§ÇãÀ"?wícõ5µ8?hyBFlò?e±ƒ!ˆgú?ßm47¸?r¸G+ýý¤?îïŸ}y?¦¸£Ðù.	?Z%^þwóŒ?o^Gé啨? <Û¤|Ù?¦fMÞLt?îØ–´?ù(M损?ÕŽªs‹?€àú/?œ¶Âȇ±?‹ÿ‰]m`¯?ïÀºðT?ff.©|ãÆ?W|²üÄ?E…ºÕÇí5?zv"µÑL?d!ISîƒAGN4FGL J0923.5+3852¿ÃvŸ»éòð@F½inX£/À9ÛýåsŒÀÀ<"æu@V¢NÉç•@ß09ƒ¯M?¹¡®æÝÅ?ˁR:Šj}@
¸e6»~@ÕÅCìi¿ÙÑãl'¤¿åZ:8
3¿è›!>>)0¿ê'?_†¶¿ïÿöût€¿Ênà]xV(AGNbcu3FGL J0923.1+3853B2 0920+39?ïߍæÕY?ftØr¹?jDyzg?d«Á˜Eñ?JëáÊÐLà?@çÊE
2?ïºk;ûj?|Ÿ'e…f?[E½·û–N?eKõT1è?{ùé¥|?t²U­O'µ?îÿ'Ø·Î?"íΗU±2?'ãGÂÊ0	?>Å¥ "ß?ŠozZeÜf?ƒ9·kB—u?ï»ßfyÓù?]gFò•ü²?j.L—ÓÞÉ?O"r‡†BŒ?tù&~»8"?UžGRHÒû?ïÊùó÷^?re¬5â<Ü?u]Ò/Ÿ?p6ÉÙfù?T—­&°k2?S­[ºP%?ï)ŒÊíéA?—z^ἡ?p}T S?zêŽ@Úm?–¯™éO?"C²®ÔÄ\?î7k÷Ÿß.?* l»wâ?¡7Aúe%8?˜Ïš¤´êS?–£ýÐÕÆ?ŠÈÀFÙ7§?ï÷5Dõ?'ÿÑP¦öÎ?ŠäœºDæ¸?u¦kéý@?'nË!Ï?z9€Ý©0AGN4FGL J0923.5+4125¿Õ×ã%\d@F¼	ԕ+À9"+¸ënÀ<i3—Ý÷@QÞc£"@xAàu >?®<ÃÇ
–?²ºýíV/7@÷×ûÕ@
òÍtg†¿ËæJâ§T˜¿ÝOÍ¿å×6èÊYU¿äe8Ó¥"¿æÿe I¿ìÃßâSGAGNfsrq3FGL J0923.3+4127B3 0920+416?ïêÎêM*?Vº+é™?5{ã±Ü?$ð¥yý'?bTÇ,¤Ï?U"ümh'?ïµXßÀ‹?}²6€š?Y¹ÀS3X?díÂړ[}?~åÿw¸?v¶4<m"©?ïÀÔN tj?l­çaªI?Ty¬Uá©?C+9˜‹øv?zwmêP*º?kv'ë]-?ï¥nžT{?bG<IóA=?xëðâí?XhbÞ%H'?tŒòäQ¹?TÁ±^Þçê?ïÂãsœÇ?s
yÆê?I´?*îÜ8?@=úM†-‹?{W¾KãTå?r©#;"?ï
¹¥©?š3SñBÀ?qˆé¤›»?|XO ôÑ'?šE'ÞD®?—1GùþY?ïÆ§CÑ;?{i¥ZŸR?b-DÈ?c;Òü(:u?‡ƒæqô?wĤܯ-?ïšá9¸«?'#¶µ~'…?'Ę+ø"Ë?wzí¾«=-?‹g_;£?tÿ}ËF3AGN4FGL J0924.0+2816¿âÈFL.p›@F7ë¯#dÀ9î—ÁREGÀ<zãv\}¯@]ðáy@.þOü—–?¯‰N?J¿¦&ú?̞ª?ñlj	ÿ]@A<%J<d?îŽÃ|Áò¿äÒ8\gà¿èÐ"uE&¿à×J4¸¿ç>àæ_E
¿ä+"XÖ[AGNfsrq3FGL J0924.0+2816B2 0920+28?ïùl~"–·?J7k?Îù ?$YÄ¥Š‹X?nb«"8¤?E7•f5ž7?H2ļ§e?ïâÂ¤Í Ò?m7s®~P?;ÙrÞßȪ?Ho¹<5ς?iÂ,ìºVg?hÄo-Ñɳ?ïºbO^¼?v
‰ÉýA?RpÚÝÃ?@¼ŸÁ¾¬g?~2ÒD@ÛÂ?u»™×«šÇ?ï÷'.ïŠE?0?¡î?4×t$Æ5?çŸüxÜ?GOŠo˜³Ò?*Çà0a…?ï÷àô÷ä(?@úr»
}W?'솠 xv?Ü÷8Á'õ?J
¼ÿrº?>]ês?ï•Ý'ô÷Ê?Œñ'«í9?Q3'VÛ#?]ÔÒeJ*?ˆbC­Y?Œ%ˆÒVa|?Úl-â?x4í<ÿÕ?]^ÑÊHC?Yï!™Ù^™?ˆ3ï*K¬G?v†Í/çW÷?ïåtìf;?Rtl«¨O?RV•h}‡?@c?a|è+u–.?LJ÷©4AGN4FGL J0924.0+0534?éaÍ.5aP@B#Bþ'Q~À:ô'ÛçÀ<ˆë"²'@ ,üÉÚ¨@â…Ãù¿t?©Ú—O¿¨é#šŽâ?ç·4Ã@	!'Ë?ïœd…D¿é᦮U¿ä³ñTk'¿àÏ;<1¿Ñ[=E@¿áãXàÿÇAGNbll3FGL J0924.2+0534RBS 0771?ïsÄÙõeƒ?¢SsY8âg?Wšƒä¥€^?Z˜}	Ìû?
¼ˆf"?¢'=A?ï›ãz°—¯?ƒ)çaMúÁ?^ôP£Vx?dÅ%vw¤©?…(—9G=d?€\''e€?ï[ÅʾÄe?€' Péa¹?^äóÊ™Ý?Eezƒ?'˜÷bk'È?€Lh–õØè?ïc'š1¼?qnñã"GÕ?aÛTh!Ók?I+'ñ$C^?'_±ýyÏ
?q jl²g?ï:Q4¥ú?'0!1A?ff¬µgÄÍ?Y©|tœª?šKàCÆ*&?'uãҏéÉ?ï$@)÷ÜV?–ÿ†Tå¬å?cÚ^°b|ƒ?mfý ºÓ+?˜ü®ó»&œ?•`"äàr?ÃýpY?Ž.Z
¬d?g8þí¼÷?Z3›ž°A?¢ÑsÔÒÄw?3QýRðv?íÓPw;˳?';@)	?|Ç綹4G?lÿâÌZ
‰?¯1û—éÕÂ?'í–ÈŽ7AGN4FGL J0925.7+5959¿äKÃè%ã@E sÞ-èÀ;-Ówá¹À<àì^b‹æ@ ¤|Ö?þb7G"ê?Å1®ù¨"?¨ËPö½Œ?ä8j¤ @"Zî?ïòÆ@Á'/¿Ö–"'I¿¿á´b\Ô¿á[þ˜÷³*¿ÔOd!ȿۏ²tƒàAGNbll3FGL J0925.6+5959NVSS J092542+595812?ï¶yóS?sižwú`w?Dò	b«(ê?3Ë£'+E?b›:4ƒ?ròAË^è?ïÊÂ`Y©a?p¦s«v {?Fìù̐0?IËۂqbŒ?wÁ0£j4ž?nsSg@¹?ïmÎs.æ?yϛéùÍ?^0duÅ.ì?\ü£þòÑ?zßâV¶k?x¼ã=ah?ï°iÂïÜÐ?a†å•y?ZØéÊaH'?@ƒn€Ò ´?€Šr'ôñ?`¸'YLUÑ?ïsD8ƒ?¿(jq~Ä?T:3#¹-·?Dú:mÑc?\Y§yÄ?">36w,?ïo§L[?ŠTŸÔ#J?TÅö¸Z.?^ë$ì'?Ò‹£mË
?ˆ¬‹cË×Y?îÄež{'Ø?ªg¬®í?d 9_^íœ?TŠy­v^l?¢o¢~‰a­?R™Q!?ï	HÊù?}Ñå8Y?p™Jø¢lÀ?^d¤ãƒVd?š¶"0ݵ¬?}€ÿ‰­|FAGN4FGL J0925.7+3126?ï/{BÁq@F­"àÀ:…¥>éIÛÀ<«ªïê@VÿYfú@ƒ¸¡œZ?½‹.`ªS•?™€È½H X?ÚæÞP­Â@'4ð!»'¿ÒJÎZk†a¿àÜ.1k³¿ä±3¼Åï¿ØÞd$í ¿çáӟyØ^¿äWŸ#FVAGNbll3FGL J0925.7+3129B2 0922+31B?ïëÇÎ$)š?O=AWåæ?A¹Bÿs†?0Š¡ö"?_"ÂY!¶?K^»sO2?ïØJµ8?qzÒ|4¿?Gq‰}Ês?Qiw—?pìtRMWß?ltã4æ?ïà1ž?pí;óšBÁ?^Õ攲žµ?Vk÷:'ÿ?‡í=êù?nUAqUªò?ï˺tkÈâ?SÑOS}h$?cHÔÕæÄ?C[BEúË?p~[b—Èá?MV+µ;û?ïÖ>öY?c5O7‹µ"?R›Ñ% Ê?CÇàÜ?pZ"Û€÷?`ФrG?ïƒÁòdr,?‹9íN²?Y¾@:ØA?c¿Aº÷?‹ë˜t`?ˆ|ù÷E?ïS֖Ð?'þç"wÇâ?mJ'ŒÓ	í?b¿œÓ ;?™,@>£Bª?&¡ÿ?ïqÃü'´?qŠº¡Û–A?z°€š%üÛ?a7
W˜ªs?†6À£¢Â?jˆµ$ËKAGN4FGL J0926.4+5412?àæ>w
@F	š¿3‡À;wžYóÀ<؂ ×@ 6PiNù?ýÙ¤K¤CA?øh;ӕ¿?²ÛóÚ­¶?ðÁàŨ]@㉠þé?åë¡òYN?×_×Ár{ž¿Û·¤F›ÅÄ¿ÞqIþ7(¿ã ®Ì0ś¿ÕDzãíAGNbll3FGL J0926.3+5409NVSS J092638+541126?ïí§¥mYÂ?JìÎqZǒ?6m	ò?"éÐa"ü?_r^ëh†?Iù ¥‡{?ïÙIµ€ªà?pç>?Bêfq‡?K~nÿÛ:
?pýâû¬™?kYËR@@?ï©~Ûl¹?eod?VYLO¶°?=ñ.ô¼­S?'Õ±ÀË?dM qx?ï§Yð® ´?_©™~óÑ?i_¯æ&­ñ?I à«4B"?£/­]>÷?]I°ß™¡?ïân²eBz?X
]½ÿŒ3?Dqžu¯?3D½á_¦@?hu&µš?V(€™ñÂË?ïxÞþM?Ž‡½_Wº?W
?/*"?a›£Þ6ĝ?ŽæÓç¦Ëd?Œsæ–G`¯?ïbµ(¸¨J?z01kríÆ?`@)7r7I?Mœyp¸R?'¡UºAá?x`ÈNÜ.±?ï!®%—¿?zZiݱ!ÿ?|Ϋ]2({?džÏù¦ï?–ÈgDø?xw6&‡p#AGN4FGL J0927.2+2454¿ëøëâøÄ^@F2wpyåŸÀ;0èÈ«ÕÜÀ<½{µƒ@*Wú½ËÓ@ ߛÜiù?ÑÁ‰7Kƨ?Æ#G'Ëvá?ó6¯Ž)ú?ù†ßúüá¿ïØgHðŠ?ïÿ¯"AôA¿åŽvàÜú¿ÐèkÄt8·¿ïûÆ«±Ê¿ãì5YAGNbcuMG2 J092720+2456?ïš@G¾z?ƒj ï\™?hÒ(ªŽÌq?d'I LÜ?ƒ;d–H~?2ˆ\À(Y?ïB
=4'­?'¶IÝ×}?|wÖmá¥?ƒ¨KÖõ	? Â¸àó?…;lëCc?îñ×HQ?šZT"úE?‰ÙöhíùD?‡¡¬xô|w?¨3Dy¨?—­Ò>×ã?îK£ºY؎?…ސMþ?›¦J#‡"?~û`ï¾F?šå>ˆ¦Ø?w`°5'®%?ïTþÎÁ]?'h"½ƒGŒ?{†—˜Ì	?t!^\Ê5å?•s¸Â%jM?Ž}	@¢C?íâˆ÷Ç¢?­ú€Äs}?žùèªG?™ÄµE)|g?©‡óŽ^{V?¤ÆG넦v?ìºxë_p9?¤'O×?–ˆ}ºq‰?ðo'¶ÿ?´Š6òUT? ©åܲ*Ý?ìt!vê?ĬÀÏ?©˜»u§ð÷?–x%;ßæ@?¯%âu}?'"rϏAGN4FGL J0928.1-2035?í»¡ÅsMf@5x¦—®ÞÀ9þç×NlÀ<c$—Žý^@ÐOo õ@Šúšeq?¸pÀ\Àº?¿å©érö@Ò}{Uá´@ºÉ,YOR?ïªFà!q¿æöÏՕɿçAȌÌ+½¿ç€Ú")=¿êï$°¹pÏ¿Ò/)"ä¤AGNfsrq3FGL J0927.9-2037PKS 0925-203?ïë~¾vf?Yëm‡§«?B ò&%Ò¶?AtT
I?_²
©O7×?T€•<kÙÖ?ïâNJe¦?m …@¦F?C˜åñpà—?Pèì(ŒÚý?hR;çÚÀ»?gJdt–!a?ï«÷NÍåÉ?vfÝG?b®q2]*?j²˜pˆ)?€V(}?qƒªÿþ?ïïã­9	?>À;û
h£?D£»Ž0±þ?(§%òæ?WŠZ–Š?:'–CZ_?ïÛçAY+?b}Èþm ?U]<k
€?M"yS'?ijIƒWg?^sKž†_Í?ï®\l<"0?†ów¨8l?W°{l4Â?hî'd¤ê?rՇsã»?">"Ï·?ïX|€¯ü?…±å¢Çñ?nô£F¿?ož•@<ZÍ?' ì
H­?'k¤MÝâ?ïË8$V?`âIƒÓ÷?`>™0Nº–?GF²@óÁA?rD¡+ž"M?\ŠB*FK{AGN4FGL J0928.2-3048¿ÕH΀V&¨@,éáŸÂ¨‡À:Rۗjë0À<(<˜6Ã@,LÖGtß@ùúÊ9?ÁÉõA‹¾?¹Q"º•?ö]‡ëlm@¿!"µ?à7Åü-ã¿å—Ae%Ç¿æü¥Øl=¿é6sXg¿ßc¼ÑG¿ïø*ÿ2$ÀAGNbcuPKS 0926-306?ïÊì±'?msÅ©bÿ?JáíWif?@K‡µù€¬?wF´â Ï4?kD‡d$ý?ï}ºoÊ_­?'±" KØ?`õ$)_×?d…rá™é?ŒTއ"?'$ÄÊ©?ï‡ã¼Ûñ‹?|t*%˜Âæ?dÑà ÿÀp?jÜ\q£æä?ˆÒ˜žý	?x'J×õãÝ?ïnPÿ])?f4W<L?d¤WÉyµë?E1ðõ<ó?Bª4÷w~?d—|âí^1?ï}›"tà?'œÏØo=?[¨4?ŒWÉ?RèM(J¢?$0áÊ4í?Ró#Äò`?î¹DôjZ?§Êù&á¯ø?q&_`á§?{c½ížm?¢FäÌåú°?¦æýb‡WÏ?îò#8GÖ?Žfêœ{'?u
î—+7?rÝB©†kP?œx"3X2v?Š¢'mƒÄ¤?î/e&†´?†o뗵‹4?€pPÄ?iyžÕ€>?¨í§×9?" _¶'ÜcAGN4FGL J0928.4-0415?ÖzFÀ%A@?Ü_õHíÀ:"a‹5RÈÀ<oÙzZ91@vœ#·•-@Õ;f›Ö?Æ˃ ±P?º8öLÖó?ñÐD¡À›@	¥ŽÎºb½?ï¦pý™s¿ä2î4%¡z¿çe`!Ràø¿æc¤FÞâ¿ïÿø]ˆò?ê/†€b;	AGNbcuPKS B0926-039?ïíh/yã?RfFô™º
?=f"`'—–?/hà`?]Ö;ǀ?P«;NRýã?lZ
_?|캅!êm?Z²Ø'?eè"6Tç?z³N1|»?tVÒHÕ?ï¬b~FÏ??sx³å‡7?a*tŒ0²Ë?f׺êíÊ?€œÃZUŠ?o–
t
??ïÌƁÊ?V½àèæó?]ÝÀL¥6é?A·-_º"k?r%O<¢¡l?QeÓ©íÈ?ïÛs&Eí~?fc¦pR/›?I.lÌ`?@-^>?nE
û0B?dâØ'úêõ?ïBwb8É?"eßâÈO?hlN"?rö(¥`ƒ@?"­Ñ"Îx¢?']VQ®9?ïdfêÎH+?ô7Kþ?n1}hòðë?rD܂¿8î?Yåü(?}"KÂoR~?ïX"…ê?wmÁX3J–?vu›'‡¥?bL9:‹?ŽÃ˜Ù[¡?sBÉ´'"AGN4FGL J0928.5+4048?Þ7ŸdÅã‹@G7žYò»À:ÝҜ¦šÀ<Âc:aûž@²Pt·?ÿÆ.¢<Ö?ÇYü ¤ü?¹1ÀíE"2?òB¸ý/¹@ z~¡Eµ¿àå´àFý¿æžã…uö¿ãk®Œp¿Øåøƒã¥¿ářœô—í¿ïÿö$´ë/AGNbll3FGL J0928.5+40481RXS J092837.8+404858?ïß´E
ó€?\,"!Ëm?Fü|i(Å+?8ގ)õ?jŒ›ß8?X¼cˆdŒÍ?ïÑð—Ïa?q+ÞÔ®çã?HÙ¶z~+6?På=…<W"?sìÀ^/°O?lI>-ÔKâ?'X —?fRGï,œ	?[ü{ƒŠ?H" 3ÀÑ?†›ËðPVý?c¯½ƒìѪ?ï•Ó÷cyL?b4~3?i[µ÷‹?GÆfözø?"4B)"?`ÜÜk¦™>?ïÃa¹$ñž?oÄ™m{æ?T—'hÐ?ERL"J\4?yMý–²¶?mUü?ïmÓLe*É?‹÷Ôzz¡?\Ss8€Ä?e¸ãy»D?€_>‡'É?‡ðŽþa?ï@%ƒŽ?|ҟÌB÷?e~Å|OG˜?T_DŒ3˜ö?•Kvñ¯øY?zš"âuY?îÒ$€p†X?€‹lbZ?Uê+¦!?eàÄ7¿?_?öÚvàZi?—Vx#©†AGN4FGL J0928.7-3529?ãÍúR¹X@&p4 ½À:B ½å©=À<0d~.Ú@<gm!–~@ã`ݐio?»»žÕ(ø¿cD§"œi?¤£áÈÂ@ҐöÝÂh?ьPû"¿èKƒŒÚ¿â`c&¿à3Vn¡žK¿ç/Ë¿Üyh¿Ú/\#—^×AGNbll3FGL J0928.9-3530NVSS J092849-352947?ïaWŒ•
z?ƒ^ðV6éÜ?d
•aÕT?R´èÏ좺?'S[ÑõÇ?'YOɌ;?îOÈ՜T4?ªC^9÷;™?i"@UOO?oÉ>'¤òW?©j2¤!Ç?©xÕÛ?îÀ%'4í?ŽÍ1Cm?v';)l?lB
uBO?¡;;fô°à?‹³)_5IØ?îø÷æ+±?q—í
D¨'?wwiqk?Sµ-ÿV´°?›=×
?oj«â÷Ò?în˜ð//?…>M*›®?~;ß:ß?qX'ë‡Ãó?¥R©~À¯›?›kÕ|r?ë9ä°ÌÅ?Â%e1CU?{opÉ«?‰ïä­Ìµ?Áœêÿ4K?ÁÕ"5"æN?í8¸êÜq?Ÿ+³•¡Åì?…»hY,W|?|+'Hä¯?³'˝?œf&£Îhé?í2Ûè7{?Š0=Þ¨"~?.cAx-T?qFÓûG?²cPÎ,Q?ˆ½Fª°ÚAGN4FGL J0929.3+5014¿Ú‹þOj0@F¶™÷LÀ9Û~@w¿À<%êÅÜÃ@/Y­€@Ê%Ðt!?¥C'«¹µ?¢ó~½JM×?ûæ8^_
@ò{PÞë¿×R]šåÊ¿Ù^ØO·Î¿ãž"jc ¿á»ßá§z¿ßfÚ?&0–¿ënxÿQæAGNbll3FGL J0929.4+5013GB6 J0929+5013?ïÂ󃁛?°AܗÂë?Z­É+I†9?'të)'m?wÚËæ7té?§—À¯Ö?ïٓo3©?l¡'xë´?AôUfCOu?Jæ^OµÚ¡?p÷½°2ý?h]âH[ü½?ïÃÚÄBuØ?m'%›‰ÍŽ?Tqã^ìïâ?]›c¶&ž?xö$ú«@W?h_Ù?ï߈^¼V'?Mߙ7Þæm?PïÔád?2SjYfØå?hÕ{Ž–?IXsÃo?ïžâˆ˜6å?­¡íã¿?ay,PeÕ?ˆ­Ä_E(â?ƒéÊPO]?§£}bˆ?ïy(ü´­-?ÏÑ&2J©?X¯ËR'è€?beØa¬s‹?ŽŸÇc´ãÖ?ŒOeW?ï}"Ol?zùp3	¾?Y_°aý¸?WÂÙ¿¢€?…t¥Éq±E?x¢ô«Ó¯?ï¯L;öXë?jÐÖ>y?eëìÇnâ?RY†ù=Ìõ?}cë l-?ežIÜVPAGN4FGL J0929.3-2414¿î¦ÒîØn@3/ÃøôõÀ:úù€‰þÀ<›>»&²@~¥¢fr?ýTq÷" ´?Ô¿""Æ?Ùè'¯qr@  F\ä@b35e"?ï¬LŸ?ö»¿âåAã¥+¿Ôy;U@¤¿ã¸ÀÅ­¿åöü¿ïþöë"GùAGNbcuNVSS J092928-241632?ï§Ö£=z?r%uÜ®GÎ?eþÔbÁ‹é?UsoCpÌS?€Š¡ÿ ¶t?néÑb,HÊ?îš_m´õ|?¢<FlËÛ5?ŠV|àç'?‰€µ6À?ŸˆÓÐV'?œlƒÎ3Þ?îè±²ód?HꯪµÈ?—íy—ÿç?wVê´§?šÒÞ:±¢?‰¸<(e?í<(Y‡Ó?†ٚþƒ?'¶žÓŽ^²?pøkÓ5C?±±¹¶ª?ƒVLÚ¥…½?ïB®aõ³?"@žöæ©Õ?|­?'^á;?qs´Ž¯´"?~ãä*1c?~_%Œyóþ?ì_²"ø?´ÆÑã?¡Fµû\Ô®?¢zž ¢I?´d"u+ai?¯ÓíbÐvÿ?ííW¸½e?™h³_ÍÌÐ?q÷e½ú?†rvŸk+?©N›–0?•eÀÆ{œ?éYvÝñ§? Þ F•>?››ê©BW?†Ô¤nbc?Ç&§1Nu? "áû)AGN4FGL J0929.6+4621¿îB0×cS·@G
 r~À;"Îa!ƒÀ<"«ùiä@þžl<>J@|ïÅYb?Õìé¢Æi?¿·ÿãz?ߘ¶…7·Ò?øSƒ""_?ï£XK±¿èo~¹Å¿ã?æŸÜ©º¿ëBµþ,Á¿ã.¨TGñ¿ïùm¿¡9AGNbcuSDSS J092922.75+462046.4?ïÌOX¥*?q|'›.C?H´[Oõ?DÙ)"ð‡k?vÁÈ]aÿ?pwypp¶º?îùeä?œ|ØP‹1?€`dÂ=üâ?y¹ì¥?˜ž!Â&?–îwA$?îÕòyÉ^r?';æR]Y?ˆSÌÁö@J?ˆëI–?™Êk{'?ˆ ¤è¼ž?îrýop¿õ?'œ¶o>Wy?‡ÉöÐù¥?oͳýà?£ö‹?Â@?~G7Û܄?ï\]‰¦?Šê;dÞe¡?b9£µ?a¾ßL¡ÜC?'-.3"X?‰ndÅN¹?í
tŒˆ¨Ê?¶'}qhû?"ÌÈX'ü?œäÝf'Rò?²¹)"m>p?²êÖoó3è?íÅÀ=àÇ?™"Á¯ò¨?"8n@te?'‡·¥æ\?©‡Ç˜²\?'Ê;Ø0HÁ?ëÇÃ@?  ói¿m[?–N¼°ÝÉ?Š#³}4Lý?¼@~9/»H?œpÜåÿiAGN4FGL J0930.3+8612?éùó¦LÒ¹@="%¿­)™À9h›WûQÀ<Eyõc¶@MßÇPa@–£E?¶J¸ o÷Š?¸y/ýÚÇó@u5'Ì÷@ˆ¿6Œ.!?·ö*NçD¿ß·RDËâ¿ã7³`<οá²+–†¿¢¿é?qdÇ)ö¿ãcBZ£‹AGNbll3FGL J0930.2+8612S5 0916+864?ïòIâ³O4?H6ýµs/??Y›<dÇ¡?1Œ½]&?S•ÓC
û?B8«	˜"œ?ïÖU0Lè«?q8W#A<z?MS!S?W`òÜ?q+§àµ\?j´Ý£?ï¿ýÿĮ?o ¤ú¥=?[)y²†Ã?cx's¶¥?y6¡ÝIï{?f&´ÐyÑ
?ïÕÆ ZJq?RB‡/zê?_H¡óoúÀ?@
påE4Ð?j•n$šB?MD1¢âî?ïâ }ÛÅ[?b•i•b?T$g+õߐ?L•UšAÜ?cMNšžM?]Ì.É|?ï'Æùf‰?…Æ.ØB'E?].câEäu?gâõæq«?‡è­þÖ_H?'ša;>z{?ï'Ö«ë?}ÌGȔÏr?ho^AÎ?mÌ_0¿5?†ŸÙ{f:¸?vé A R«?¦á*Ó?q,ûÓò?sf;xpþ?]jÇj&€C?h8ŠmT?iƒæÒy{AGN4FGL J0930.5+4951?¦ËÄG/N@FØwîN&ÕÀ:ÌÉÀ¨ÒÀ<È±µR@!t1¹áb±?ýP2é?Áǧ‰qX]?ƒMŽF@?Åö€û=" @÷ŒV:_¿àÕ¿ðEwÙ¿ä<ôb=ú¿ãooŸ?‹¿ß2ù<†ª¿Ýnm[x Î?«Á^¥…iAGNbll3FGL J0930.0+49511ES 0927+500?ïå¹ì¹Z?VÈZ¬†Ì±?9é'¤·°Ð?&ˆ.2"ø?g	Âë²I?U1""àµ?ïȸ°áï?s«c{9"?G4Ëê£?LÓä•áq?xÀàòQù=?qÝó&ÜðR?ï˜fiҒÆ?t¨»¤ŸÖ?T¢Ðp¹…+?>&‹ƒ³ü?‡R†3å?t÷2,?ïmµ?rY½Ââøç?U? àzöŒ?;(¿–})?ÅÀô9i?rŠ™¿Ç?ïÖ¡§?dÝÛEì?CëÈIÖþ?3JËZ¯ŸW?r|Ím÷ùM?bå¢ð$&»?ïj‹;ÝÑ­?Ž²•šÚ¬÷?U"›ÆE¥K?^ØðöFx?'VNÆU?xOï£}?ï.¤Ç[Yÿ?…S$f°œ?_íNe©S&?U«ëN?˜,'*¢ò?"œ™¸ª)T?îAaG X™?'žvØaq?o¢ª"Zï?a}ÄF®t¤?©ïÊÂuIÈ?'²¿å›–AGN4FGL J0930.5+5132¿ç¼j-_""@FªJ¾j3{À;¿°ä8úÀ=u=™¾ƒ@ D߀®'"?ü¶¦4²4?ҒߪJ?Ïv³»ƒÏ-?ûtÓçsA@@¶©
оt¿ßÓ^Kå± ¿ïÿ\‹/ô?ïüSme^)¿ã;§««¿áÓÌ/îÛ¿ïÿþó…õAGNbll3FGL J0930.7+5133NVSS J093033+513216?ïHƒu?¦3ók‹?S
äüm•?VAsfÎÇ?•½Nú"?¥Ò}{Uá´?ïx3BwŸ?"W©Œç;±?^â0$Î?d4|SΌR?"àï4#õ³?€ÿpD×ç…?íÙ2Kà0à?¢ö©ó…©?tor÷Oé?z?è9iª?¯Þíû—x?¢M
+€v?ïRPSnUã?wtZ͊]?aGò~2Ó?Så^à R?"Œ÷IÍÿR?v~G¤G?ïäR´Ù?Ÿði¶²A!?b"zK˜«B?Zšñ뺭¡?Q²½'w?Ÿ–þœ™!{?îÞSo¾©É?¢St6ׯ?o(½ÑÿÐ?z¬-Q¾)ï? (=&u6m? wâ]Ú[?ì€eŽWÐ?©ÔûœþYá?}ÄâX1gÕ?4íC?º#¦«ÙjÈ?©ÆY†¨'?î*ÕMœ7{?•²ç®ÿ?kHw˜à݋?g³iՀØ\?«ž#®:Mt?•IéÚ®õ'AGN4FGL J0930.7+3502?ßåë¤Ò@G`ÉÀ¨ÒÀ;0f('ðÀ<ܾ•Òd¼@ÜY·Vmö@+À nŸñ?É?æPl?­HPÑ©«`?ã"cßùOb@î¿æµ?ïê"Q€ü?·ÌZ ²Òü¿æòƒàÊ°"¿Ð]ãŸ''¿éÔ+{¯¿ïøÿ?æŸÝAGNbllB2 0927+35?ï"%{å~Ÿ?ˆÿšû$–;?aEU}î?UÔëÍîˆÓ?Š¶_os¢±?‡ïÖ7Óá?ï¾Sm˜èL?x#•=?U|=¾Ö'Â?]€ïd3~°?{w9¼÷(?s'Ñy[–?ï6#×þY?…Üϵp ã?qž+•€=|?j
Õ¿
Qž?"ÔyDރ?ƒŸ7͘(?ïV,Ì*ª<?pàøg€#?"¿Ò¤ŽPv?e.ö´û?…´úMW"s?dÒ}·£`?îßq¢"¤À?– rá$ñÈ?q‡<öY¦Î?fñ‡QýÖ?Ÿ¯üxJG?•˜‹m*&¤?ï5 Ù>u1?'F^šP^ù?iwÞ^ž´Ÿ?q"M•.¯Ò?–,é™BS?‹ëì¤c?îyùeSŽ??"ˆÀ°†Õ?~Tn‡?v*åZËÈ?¤œ†`'A/?'d©­ù¿?îQeÖÒä?‰l¦XB,?™aÂäçW?'ÊÔòW˜:?œr2[ù¤<?+ˆtÑAGN4FGL J0930.9-1015?¢DáLyî@<µ?á—_-À:Z'¹hÀ<vö=Ÿ@æF×)òî@WUÿæՍ?¿]ç;ãÛÝ?´zr!…‹Æ?ñ+!Z³@ê$O?®?ïÿÕ%t.¿ÝÜxüÁE¿äŸNyà–®¿édŸ;ïð¿ááHtEL¿ïÛþ~ÀAGNbcuTXS 0928-099?ïÊ)ѬýÇ? °tsç¦?2ˆ_y?{î?T› ÏÍ@?y'vSX? 
÷¼2Z?ïçJÓý‡o?h	®ò÷¥?9>¹ÂbŸ_?Eîbv»?eTõwQJ?d_#³WÁ?ï€}'ëMä?†¦ÿûѱ´?`ö«b'ÍÃ?oq¾•ó¸ò?‹£+ƒñ¥?"ÄÚI"ñ?ïæà+Ï;½?DVk:ß´?F\á×
Š?)"ƒ+Ïù?cˆ›í¡Kœ?A΄®=ú?ïÚö"š§?qëU¶ÜCº?8QØXæl‰?-XzÀˆº}?pÿ˜›©©†?q½´J±¿T?ﮛóªËà?Ý¯ÁÓá?P'á
µkû?\ˆöq~wö?'F§¬Àw?€/ÝÝÓÂ?ï0±"sP?ì{$Ôh?h~ðtìl?n"úNºÌ?–ý™ðÂÐi?Œòђ[9?ï·%5$ˆ?cá·.?_ˆN^Œ?HÔќZœÉ?|‹^ÕçÀQ?a°×Èÿ8AGN4FGL J0930.9+0033?çn~ù¸Æ¹@AŽ'bEoÀ9›õœÏ®ÿÀ<G^ñýÞ¾@L°·mj@Ƭ!\?µKÌ ñÁh?Áö*¿@ƐšíV°@ÿ÷ªÖ¿ÉjW·¡íP¿åþŸ­¯Ñ¿é­'©èò¿ë0߁w^¿ïÿØþ3w&¿ïØAªÅ;AGNfsrqPKS 0928+008?ïá"ûZ‡i?`†N–lµ?WötÁ™?PNüÂÃ(ä?bÊgL'f?Xö>¨Ï?ãpÜ?ªßÛÈ=F?'fôß?¢'ž'
"$?—×Éýzï©?–~ÑÀr8'?ï˜d>?%_ÌHŒo?pZr€eÂ?xlÐã²Â`?¹À¹—³Š?uÚ¯0L??ï»BX6š?}ŠwïÑ
Ö?"5Ç{îÒ ?yS€ñ-/ˆ?å `6¼J?b"ŒÙãþ?ï¸OUŽãï?u_î)¢;ƒ?rU'1Œ.?qg¾@E'?qÌÿ¯U?dÄYJnð?ì°511©?¿ig"•ó¿?¦ZMÏ!Øñ?¶Ê9÷3?®¢_0—~?¬z‡&A¶˜?ï)ńÀ)â?óëqö?}v¢Á
¿?øaú"¨î?"i¦·ºA?"ÚvSzm³?íUÙèáwÌ?ý:n_ý?®êÄ`è?›Y}UÞ\V?—p±Uédµ?…ÊvZ¡AGN4FGL J0931.2-8533¿ç_Չù'QÀ8:dž;îÄÀ9ÏÝ;¯ÙwÀ<H~@WZ¶"áÒ@6Øôù;Á?´4T_AÉ?™òĒZz?ã[é4â`@Û3¡íûñ?ïðDÁPï¿áŽÉý³ø¿é•lä.é"¿âÒ5!Iü£¿ê';ÿŠ;¿ïÿÔ@ßn:AGNbcuPKS 0936-853?ïÜ8—Š?yÃΓüÃ?BòëCú\?5™îØûNw?o'l
LÁ?cÜ¢=¼?ïæÈbJ«?kûiù6ú?4¨#ö®`d?CÞUPãt?f¢ä÷³ü¬?hâ7§;	Ã?ï—Ö£Í?'Òüfkc?d!o…V¾?o¡Íƒ"Ÿ?…û\÷	´?|î8öV?ïÜ*h¼ày?P¦î¥:eÅ?HÇ{Z.¹æ?,pñr//¶?m£¸š{lä?O*,I˜#?ïÖْÐI&?kÂÕ5§°Ì?S¶RšQ.'?H¦;âtdQ?oKD(*ï?h9j‰¨Œ.?ï¼rͅŒû?'LÞíA$£?E€Ñ'ëÝ?[Q˜óâ)?m·‡?€ú¾Â†ïf?ïgZ5fÐU?ƒÙt_'IÇ?o0ÙëÇ?t¼Fün?Ž]<SêÏ?€w©Vª?ï—y€
pE?oüj¯®Q_?d¯È½n?PðfY¤)Ì?"õ­¾*!Û?lc7ؕu AGN4FGL J0931.9+6737?èÒ2"®@Cåwž™À9õ*8¸®2À<Œ
¨y0@¦Pç}@ïw݇/?²õçMVŸõ?¦ã,Š¢…Ñ?óŸÁ?/Á@
¡–‰ÄºZ?ïÿ·ÀÌ
Š¿â¿a!-!¿å1ß«Ì¢¿âß5…¿älɌ¦l¿ïmŸ`=AGNrdg3FGL J0931.8+6739NGC 2892?ï뚁ºÄ{?WUâæaÄÑ?0N)ºˆŒ<?#®®5ù}z?b[¸é88ç?V |…Sf?ïܘ»çæó?p¡<œ"­¿?Då'ÐpÙ?PW"KÊ?n-ú0R™-?kºÌ?éîŠ|?€=`qo?U8d´VQ¥?Pn­Å9d?†x8êºðî?æÕPÅ»o?ïÜc'm?Nñ")9!?^ô‹7µ_??C Œ±jU?d"µQú&?GÍm7t?ïÒ¼S5·?p·Ÿ—*E?@×Yǀ'¡?5[\—²¾?t†ë)Ö\?oÊo½?¸0ï?‡\÷Ã>°I?W-ÆóÖ?bSwj Ø?†45¾3õ?"¿h|Øj?ï`^ÖÇo?Œ³…+j?`8$õ-ð"?c³èÀh.?'øoƒi®$?Œ^ɒoS¬?ïŸ6'¬?k†c"‡:?v¨úyÊ?]RSû¥áO?zj;µq<1?cíª"Ï»EAGN4FGL J0932.6+5306?ï¥væ)@F ÇŸfb5À9¡®×€*À<‹íóŽ¶@b9®øP‰@/ÜÌõ?¯S¾Ãõ¶?µBJ¨DØ!@Â;C¢ìÿ@†Èg¸K?áÍaýËó3¿ãÑG»€t/¿æd2Dꁿ炞«QR¿è7·6¿ãÐ9h×YïAGNfsrqS4 0929+53?ïzx²vèÈ?¹Ú§^†Ñž?RÒ(»¼ØY?}KªQ
q?ŽB7,ô?¸mVC†"?ïâ?Qñܞ?ií-ˆUüÅ?>=¼2ÿ'?FE[m×?jfWLíï?eá´¸_?ï¹
oÕ%?s_˜WTn¥?Vf8Båvs?UOSq	Œ*?}ß¹ðu?r{š'Þ#?ïýJݸœ-?ÛGÜu<?!-kQiu?_x ï=%?*$´ó´%þ?çü·
EÆ?ïáÛŽy? RXˆxÿ?2G'µ	—w?&2‰·*^?kÜXÛå¢? Râ¤E1G?ïšÑ@`(›?†NŽ´3?R/©éÛià?`¬Y·AÐN?‡º¶!û?"™pÔÔX1?ïx°Ú—ªp?€ð⏄}`?c™¶SŸ?_n‹6G?Œí…5%Õ?~ÕgƒãÉ?ïø1Ó?`F?<P‰ÿ¡w?9
á—ÖCø?(¸ÃƒÐÛo?B³A•±o?4õ¶y›ñ¼AGN4FGL J0932.7+1041¿éBe¶ú8Ò@DIÞ½çÀ:ñŽd²1@À<ŸN"
@ /¤¨ìGç?ûüÇÓ¦Ü?Ì" 3§!?жIÿj.@S¥Ýt»@GmÑi¿Œ?ã[}i¸*~¿é˜¤ Üš?ÐÓۉÓÿ¿ÍøNñ¿âÝø©Êi¿ïÿ£^ilÖAGNbllNVSS J093239+104231?ïÇó‡C`?fC͂ÿÍ?Xdç˾?F§…WaZ.?uþc
¤é@?cH+niÿF?ï"YFuã»?'‹V¶H9?gIàâl?h!,x–ƒ&?‰66ú'L?@*T¡Ê?ïVæWÒÌ?Üp
A!¬?m"=¢^w?i¢iC¦·?'b›IªÀ?W­Bó4‹?î
Ea;·Å?'¡ú°Çã?"64\5…}?f­~Š$?ªNՏU?Aüvøø¬?ïˆÿ¸(ó6?{*(0?tÊ?h"*©š@?X>N[Bó?‡¸ðèY?xKÚV¼`?îÅ.o±q?™e\Û`)?wª s"¬ˆ?z³Æp±%Ï? ·Ú—"·^?•q'°;J?îůyL>"?Œ‹' ÈN?v=2l
(œ?tŠÅ"Ʊ$? Ýb z£?Š"W¤ÉÒ?ë½zŽ*i?x€ÓÚ?"$Žè,?ƒ~ۋU+?ÁE"!?ô?œ˜ÇoAGN4FGL J0933.5-5240?âM'>÷ü¿åÇòÝ؍ËÀ:Ͼï"xÀ;È$g¾U;@!B<¨§Ôp?û´ò»sÞõ?Îß$}¸½v?ÑhEƒíµÑ@½ÞÎW@U›ÛhF?ïeû7Cc¿é MÈ௿ÜÒýhv¿Ù6ªK˜"Ç¿Úó­¡¹M¿¿çÓșaeAGNbcuPMN J0933-5240?æ‡{Õ©?æ‡Ç<É?vzÄ»9\?g¿¡‡ûê£?җ!½x?Õ8Ò?ͯ¾ZTq?ÉFÄLBN?‰Éuœ'±ï?yÜ"?èWî9À&\?ÉGr°K¸?èÐÞӛ¯/?«C&Ed?¡4SÆ[?"Ø1ÍŽ?ÈooÀhv?¨ú¿"|áY?æû^ïé? .Õ)¸l5?Ü@ù"?qê"…Ÿ?Ðü¹:ôž? ò}¡Æƒ?Û^N>ýA?ÆBf!G"~?‡öaÃ)åö?{wŽál&?âwQÆX?Ætcv"SV?À™<¸©:ˆ?½. –Y"?"Š&QPê#?"F¿ag>¢?뇈8âäU?½—	±Úƒ?ዖù!ƒ?³²‰à>¿?±yðzÒá?Ÿî>!þÌ\?؊VH…!?±®õi.Ò?ÜhKøjÏ?­mÓ¥Ö-?š'$"…"?ˆç¹À´T?à÷Èߊó?­ßÿyZO{MIXED4FGL J0934.3+3926?䙎ˤ@GÉ-ÀÊ`À:-ŽÚ"ö¥À<‰ì©&¥@}ÈoEF@i3]$žE?·3Øõz?Ž8èÿ³T?ÓþzÄÂ<@É"ž:"$?ïýqåöi~¿ä\u¡Â²í¿æɨnZQ¿â¹Ùె¿æöJ²È¿ïÿø¨ó©°AGNbll3FGL J0934.1+3933GB6 J0934+3926?ïÞ`…s?ab"[›'?MWµ8ï?@ØíµÒaé?j—Ûè§~?^ÀÆcç?ïÑ~E]à¹?uf›©_þ?M{!–êD?VbMÀcÆ?s'}
˜T*?p²ÃíLª?ïS§i]^?wüG
+Ÿ?dáW?fzNî'+¢?‡*Òý'-?qG[‰8?ï¹%#Â?]tÌNwÍ?qëUϙs˜?RîçhQa?q'´"éù?RÂÿô{?ïÁuàE¿A?oÕ*óîU?_Ä<ïvÿ?QÛskû]?wT	qÊ
?l•G4,?ïrFc¼'î?ö¼±âë¼?a%/jHð?k^Ìn?(ÓÇ9?ŒwÅs7?ïÃâ²+?ˆ˜Q|Ë?q
'Qj6›?o¾<ÒËiÍ?˜\C1^ðò?…xÄÛéT«?ï7[&tçf?yÒ«uâ?Š­DŸ«Ò7?q¬äU¦¹á?‡{ñÃT<?mÜÆùd‹AGN4FGL J0934.5-1720?ٙ۱Ÿ¨Z@8ÃF4—·AÀ:åV"tnÀ<__á'@ 됚—?ÿ%"ü|?ÇÂЊ¢H?°³¢?–ª?îïŸËm@­Åñxô¿ÜÈ'ç%"¿êõŠèü®?ïþ@!Ù¶¿è³2ÇÓi¿Û,kãþ"¿Ñç6žË2AGNbllRXC J0934.4-1721?ïfw›md?‹dõm	?Nu€·x?@ç»ÄÊÉ?'=`Šc®—?‹š/à{?ï‰ìy\Û?ˆI¬ª&ƒ?dG²w³)0?i?ÅþlZ?ˆªXUBõ?"7îÌV{?ïRÀÓUŽ?ŽÏrªH?cê áå'?TZ`þƒbO?œ˜cáWŠ?Ž@
yIÉÌ?íÿÖñ$+?‹î¨iÁÔ?luµ\˜ZH?d`Â†?®F§8¦€+?ŠµÊG¨?î¢$·¼¼¬?šSûeø"‹?Zw²²þ›?M܇×d?¥	øf/J?™ûºB}öG?îÀrU ݊?¢ÕŒÚxÅ?sn{Ý=׫?¯V¤7fx?¡‹4²&h? É<!'ôº?íÈ;ã°éí?4(8žÑ?q%¾]Ï»?hƒµÒÃZ€?°­†¨Ñ?œ›Ϫ×í?ê¡žè–Š?©WA2äԌ?{î"?xŠSíÉ5?ğÎ"'?©	íÕ*ŒAGN4FGL J0935.3-1736?æOvl@8¹'^éšcÀ:GäB4WöÀ<2Ÿèh3Æ@!mQ³¦á?û®Ð³Z§?ÄoH7QOÿ?º¢žA-?üG*{Ԍµ?ÿ·Æñ¬¿ïkÚ佄Z?ïõeݪj¢¿í†òÞ€é?Öª"XŸÔ¿Ô¾B%>}ê¿ç:R ß²AGNbll3FGL J0935.1-1736NVSS J093514-173658?îâpqœ?ªsyË"Fµ?c¼Ò!k?a­]$Ý~?­Gø¼9¸¦?ª
ü""š?ïÌèÍ´î?{GT/³ž?S¤ï'/:?dæíp?‡ò?t¢]‰"¤?sæ;"r=?큻̟Up?¡&Õ»_œ[?zº¦«º&W?Ñpôªyu?²Fw/LÎÚ? az:Ѷ?îj®f?ˆ©þó7?†S
¶Oq}?twïžàŠ­?£ÂA²Á¢'?…†/¶OS?ìþžàš"ð?³~#FïD?}¯2]ÏVÓ?yl¦µvší?¶0ÖÝÆ?³§ç¦r?ï<T
²û.?™H?ª|û/?n[€èþ?yÎ1&ï¨!?"¥"1|x?•¯×ÿ\¡?ìNâZlvå?¤ãÌ\~I÷?‰äº'l?‰d)´Õ?ºLUê©gÔ?£TÒ>v"N?ëïé¸HŽî?¦UI'†Ö¿? ˜¾#ýæ>?™æ¢J"?¸4S*à®u?¡§"ˆ£B´AGN4FGL J0936.3-2111¿ä.¬QÐO@6už×ÆûÒÀ:¿YHp²À<iéæ¹@ é#mîE?÷ d#–?ǚ¶Äø˜?ÔÛ:£¿ã/@¢HåL"@E`í²v¿ïÿýF\I?ï÷{+ðHÓ?ìäS äQ#¿Ñؗü`Ž5¿×<ü_·u£¿æåÂ!øùAGNbll3FGL J0936.3-2114TXS 0933-209?íR{¢­?À†œV23?"(qÁÁßg?¢Âò)?Ï?°b
è½?º"U¼e?ハ§ŽNã?€.S‡‰õ(?Z–2ž†ë?kù›ÒKï?zöÀÙ?wüAÈe?ì#¡¼ã?©1lGDñ?¢3fZŽ'1?šIsXÀ ?µÉ>ð"3Ô?¥+,u8?îA»ŽXjG?~ðw¬î?s*pÉn,?aì¶úa?©~ù«n?Œ(š¸YvŠ?ío6</¹µ?µ/PÔȈ‰?•ÒoÒ_ƒª? ößõè]?®#dRÔã?°™zçõµ?ï:¥6Ÿ"?žáêªÔ
¡?sì´"£Å?†ª'–$?"ãÝûíM€?—(8i!?ëÃÙLü¢?¨}B¦Е?¤`±!á?›U^¿¨D?¹Iˆ¦Š?¥n÷'Δ?ìp¯ï¶¦?£ªäAHúº?~–w‡•Dÿ?x;¾$nñd?º'
›—ÿ?£aið™ÅAGN4FGL J0936.5+1847?äæ™/Dç@FR  ô×®À:®4|ßN°À< …S'wŒ@ÁÕh|Á?þ@¾kàùª?ʊÄê€;û?Ã*[]É´¿?øJÚ3½œ®?ù¥HÇD!Ã?ë£t'ˆÜ¿ê7N€–"U¿Õýu‹¿ÜžŠD<
¿ëP.Ë¿ª°#çF¡AGNbllGB6 J0936+1850?ïlÉíÒßi?…If໕c?i8–7í
?`Žhs;øÞ?Ž_@,a?ƒNFxÏ
‰?îÌD‰[õ?—\,†Ôj?ˆn÷¹.?†IB¡â©³?š@/Tˆ@Ì?©º½Åa¸?îý0'S×Ã?
{ú³v ?|vTî3lÆ?€þ,5Q?™<Zrij?‹ƒ1­Š?í¾çóU?†Ü!…Ác?šæÅæ6|Õ?x v_/Hï?¦žהA?Wdp
¢?î,.ifk?¡vzhä¶?"&]ŒÎ/?xíÔùÓÖU?¨3'
ø$Á? EZ¡7ýÛ?ìàˆ'E- ?¯"óã)??™û¢±D?š)ŠN3Oõ?²|Ö%4C´?¨âënû?îÉ~[(?™ð¤"(Ùl?"Díj[#v?4"E=•?ª,¼1Û+?—%êՉOn?꿋rSHk?œÂg9?Õ?©>sþ}8?ãìü?½djo¬Øˆ?–—pàÂìÝAGN4FGL J0937.1+5008¿ä†²?i½@GVºI<‰ôÀ:?'Á^ÁÀ< *#¿ø©@ GÏ!É@z䢬h?ÁS¬åÑ«"?ƒåä¥@+e>H:+@
žÄ½B?í´®"%â¿âÀ_×,v¿åš9҉¥0¿å݅TÖ¿ïññ\Ï¿ïÙ§'æøAGNfsrq3FGL J0937.7+5008GB6 J0937+5008?ï׿£)Ì?c¾ô³?^À~Ë%~?SXP"'Ô?i˜Úsé?\2¸¼ (?ï›Yã©»®?ˆÜ˜xw?iH¹?™Îi?wˆ82øV
?'×XɜÇ?~Y>â =?ï—÷ÛÒþ?8-µÇ)ü?h'áyåÃ?h"`«V§w?ƒÝäq2¸?zžh/ô[?ï~Ä>'hÑ?jmxòæ­?Úr¾¾¬?b£Se…{b?|èû?õŽ
?`»Ô=?ï›z>èD?xK/—´õe?tŒ€é‹Õ¥?iXæ€
>?}¶_Ë142?q;ó'SÅ:?îìyݳò-?žËü:?xÁ;>-ƒå?†5ìŒ_é,?œ@u~ág?—o³5.Ýy?ï3ý'¡ä¨?‰ë×øüŠè?ySð.‡?x­'zÌ.¬?"+Q½aõ¾?…C–ÆK@?›ù?ˆzTþá§7?˜¯Èb¸d"?€¸£·!-?"à$@dzm?}ï·lðŸAGN4FGL J0937.9-1434¿î¥ÒPU"@;7Ffìž#À:v^$x…MÀ<o»^æ?e@ 
Õö›þ?ýæD·%?Äú`XÛ8u?Á¤÷Ãpƒ?þXˆøa¦
@
ä"¬¿î¶Ãvö?ï÷uýÞÄ¿á"&ÈÁ¥Q¿à8äl-P¿×oXz™¿êá´N_ßAGNbll3FGL J0937.9-1435NVSS J093754-143350?ïàaU.±?Œ>¡án?>y#‰ Á?\3a‹öÝ?kÏÕ.\í?‰'?<‡Ä?ïåfTPlÞ?j´¼Ò-/Ë?>mþL?K—ò­¦ï?f֙‡Ù†L?eôžP@¥?ï ¿4!´u?€øU?R5g›½±·?V±ÙˆJ
?…‰…öƽ?~ɳL*Œ?ï¿%yêÛ?Zä:ø²'k?Pº»™ùJ?4Mã‡×(á?|>Îî¢Kû?YÝnOM?ïÙ'¾àÐæ?l"‰S3*e?Hr0º³Ð?Cl.(—?p]ڙ›Ÿg?j¶fúx9?צּ1̚'?ã}4ÖmØ?Mtš!Ê@?Y+ÛϖÐ?'Ç)úlC¨?€vuAfwç?ïEã•w\>?ˆÝ6xù@<?[NJ&ä¸'?\e"Ƭed?•‡¬–h»?ˆ" ½i?ïZ5âÔºÇ?vŸhɖ¯(?añÈ}‡h2?PÒ`òH†P?'{
}.?uÔg5
AGN4FGL J0938.9-6403?␚®†T‡À!AMµ•x£À::Þ¨—c^À<;0µªq@?Ôó@@˜Ž¼ÆÅL?½ÊA¤åþ?­â~ðå ?ðXÑRm‹@éØÅ~yÙ?îˆ|:䝿äžr£hû¿áV™y¹*¿çôÀfŒý¿Öý'aĖ¿æµ¾§6AGNbcu3FGL J0937.8-64071RXS J093850.5-640334?îFŒ¥ÚŽ?œ´%åÀi?fK¬•?T­»ÑÞÁ?ª6 ô"nm?œ	-Ùµœ?ì;%󄜇?±ÓQÓà¦ï?[ä¤ÅÒv?d"éeŠŠ?½·=ՉÅø?±'ŸMƒ?î³¾Hâ?'.…GY?l$߁‡…?\°¨Ëëm?£
 ‰oL`?³?uò?ïn;`9ŒÐ?h6ºãQ…?`jÙ>Þ?A·EÁ8ú?+OûE$/?gRöJá,?ëäùdü¶?²
ŠÚzd"?|›Ábó£?l´oîÛV‡?¿xÂù(9?±®M?ÂÆ`?çLcèªh?ÃWœ ÷5?hŠ…ŠÜýó?x?ß4̚?Ñ6#$i¹$?Ã,€OE¸?ì\7#â®?¤@÷lã¢	?ê2"cð|?t™x/Qý?»£Å}´G?£Qä÷zk?îELè]nh?‡':ê1˜œ?x.ñª?cNxõ'gs?¨©p×LN?‡C´RAGN4FGL J0939.3-1732?ï¶=ñŸŒo@9yØ¥H#…À:
tÓ³¬À<Yõ2F¤@œ' PíÙ@'%IÆ?¼µ¿êç!?½Å°"òô)?ÿη«c@ÙÛ]3a×?ïýCWm¥¿å©?Êjå¿áÒ¯')c¿äKùӖª¿æuQ@9¿ïèÎ?ézAGNbcu3FGL J0939.2-1732TXS 0936-173?ïïÿWl+*?NIيSqÑ?/Vt_ð´z?!ÕñžÉEb?\'wbèÑ?L°,iËÜì?ïãl+é?mžb÷$›?AQA´¦?K^Ntsùa?h–C4q¢?hrWP=ï?ï²[Oé?uÉ3˜l?YÄ.Vc?VÑTó[ß?€0¶"¾Ðî?sð±-ä?ïÙÉÖù!?P6Q!lÖZ?SO\x?38´æUÞ?mF®Â£´?MMíjØöÁ?ïäyz'?\7
½¥å?>6Yô'\€?5§.
.K?g¿ºŸáwÎ?ZNòã¬1?ï¯Hy]d?À8Pf½T?Páj‰MÖ~?`ό‡?'˓îˆ)?€?¾ìðE?ï|ÅYÕ£$?}[ÉÊ»?fæ?š3ÅB?ePOƸEâ?‹'"CÊ?zrH$7"ÿ?ï—å{ö?l#…¡Û(¥?h­¿¹V?Oý»ô?ƒÛL[<*—?i-¿LüÈìAGN4FGL J0940.0-2828¿àԜÏÙò@1éi ­ŠÀ9ùÓ°ìœvÀ<3ÅìÞ»@z[±×~@£ŽDÑÁ(?¸f¸³?ƙ˃ ±P@Mí®Ä¤	@Euà¬Óˆ?è]ÿÅGN¿ä` CAs¿å"—Ú|¸¸¿äy;.ª7¿ïþ—J4¹?Â<:˜Ø(¡AGNbcu3FGL J0939.9-2831TXS 0937-282?ïÓJ㱞Q?ƒVbÂ×ÓT?bܗè`ôY?Yðìê_?i؄Œ|Z±?'ãHsf?ïÚ½(‹Ÿ?qK/öâ"á?N@):?[Õíá†"?m¿h²L•?i³OãÄ`?ïw!-»é¿?"K'&+ù?z›ãò5?~—°ãC¦?"éÂӄÿ?yfw"·=+?ïÔ´N?Ra`"û·Q?S×bŘò?97Œ9íoÀ?qM=¯'Ç?OhŽ¥J?ï·fÃ|õ?sø˜âÍZµ?r[ªð^ðL?hN4Ÿœû?qñTÃà×?i˜\ܽ™H?âà¬Ë?ß(æ–1?f»$ ÷›}?y¾ƒŠðÓ¢?‰¨¾+ˆT?‰Zqb.M?îï{ÙXÒ?'l	ÿ¸Pw?ŠQ°:"?ˆËéºþ ?"ç¾0pn?†ªóJÒ6?ïsK–xÊ9?t'??S{?p"a²7?[_XÆ?ŠãiÓJ˜¿?pþ§'² AGN4FGL J0940.4+6148?æ|(Í~£t@Eš:э%îÀ:ž:'ÌE¾À<œl%Ã(@ ÿƒ'ǁ?ûþ FÇd®?¿[äØ1Yê?²ùÞÓµtA?ôʇx.æ@jk5Øÿá¿Ü¡]Þ,›"¿íNj¼[f¿·Ãñ®¿ÛiÝk폿æx`ˆ"?Ç7¿)ÌAGNbll2FGL J0941.4+6148RX J0940.3+6148?ïä{
×÷?kî4Yƒ"ñ?9uAK¥†?2גwы"?hVO³j§É?j@X¾:ÁP?ïÎOk£=?sI©&2yd?I+®Zèe"?QóïtAC`?u²Ô]ÏÙ?pUL9ËÇú?ïx,´M®?‡¨ï{bà?Nç'ù?7£Ã9ZK?/Qª¬6?‡›¶""A?ïˆkËní?kj,ž	'?`²r,'
&?D×ñU$è@?‰¸pŠ±¾6?jw7¢?ïÉ£^X>Ê?vÐ@<úª?JÁöÝ6¦?Aù£¶£Q?wÖ×ßH§?u€ÖB¯	"?ïjæ'4C?ŒåÊò2?[íãÊ̋Ä?eö Ù¼?äO¬ùí?ŠqÏ·I+?îî"§
ºB?•fàíg¸?WƒA/Ύ?XŸ`ÂàRL? eIvd·ð?"ÑL۝A'?î"þ'Ë&ã?‡ÀŸö]s?uKÊFö4«?dRâÐ@1
?¤Zv7?‡jÔçzÂAGN4FGL J0940.7-6105?ä¸0
À!)Es§˜À9èy§‹Ê¤À;ڽۘA«@—Š«j&@æc[ïêß?ÁEj˜?Áâò=ŸÀ@;†Eÿ¾'@	C\($¿ÝÇkäՂ(¿ÓENJm¬¬¿æ}å=ÜÚa¿ç¯žˆì£,¿ïicÁpx8¿ïÿú@ùDzAGNbcu3FGL J0940.7-6102MRC 0939-608?ï|ç¥ÒHH?"¶ïR½û?h­5Gªw"?b<f
Ý°?ŠšÉ.,š/?'/÷´ä?ìܓ.Îþ?³	r'Á#¦?fsxÍc!?pÞ¾BT¦?¸gÊÄ:Ö5?²¹ÂB=
é?îŸÖ}Ú?"
³¡5·?ƒeF#ýk?¨Öèuoý?¡B…Λ
?¨º–5ÙM?Kã*?z"^‰PµË?†%²Ô4(?c³.Gfs?¡MîÁÜ\L?wL쭃U?îËq"F
?š¼'9à"?ƒ8"'©U?'Ø…Ɛ?œõlQ'–­?–[o`Œ¼ú?ç%U­?Å!å5¬é?{ܹ¾Ï÷`?‰l…_14?шvÍwþ¥?ÄÐoY)<?íaßÑa\? 41ßñά?šªf(?‰žbY¦	v?°Ê|Šqò?›‰á¶U÷_?ì0^EõF'?•ál wŠI?žü
öñ?ƒåý@9]?¶öMs²?'<w5³Ä}AGN4FGL J0940.9-1335¿ïþL?QW@<lӝ¡fÀ9œÈ\ûƒ™À<'Kžd¶@üËÙ1ß÷@g'ûÈbÛ?²z|öê?½iIśÖ
@‰—Þ®v @¥o;¢?иœ>9¡Œ¿áŸ=ب£¿äNô‰u_¿èWÿ›V2¿çþîк˜¿ïùö€û=#AGNfsrq3FGL J0940.9-1337TXS 0938-133?ïÜÔT*¤™?q›Šæ‹E?; ³­_ˆ?1ß²pzU?oɧÍ
¸C?q•s›,?ïäIeF"F?i]R°—Þ??wþÇe²?IŸUYg·W?gǚä=pë?dÿv•™f?îàtcY?˜¤›D-p??cT¹@Ú	ÿ?nT( ²‰t? Éý'"Ç?˜Iëã;Ä¿?ïê"vÕa?CP<^ph?>hWX0N?!áEK²?aŸ‡ý2mØ?A…×ç3B?ï­òÏjáË?‡z•Í{+A?H…Jˆ?M¿¹}¿B-?ƒ³ÿä`Ä?†5Ô8:?ï¥å	"Ž?'¥õ;Žþ?T›%7ù?aÕLB¨6?ƒó[±öj}?€¨&ˆ«ŽÒ?íúý7ßÑs?¤š^°L?låUyÃC?q7ZI?®×&µ#ø?¤{\ÛUÚ?ïÅϕ݀?cßNƒ/?T?OŒ2eq?Aìjõ|3?xa^M?a¿hUìÖ	AGN4FGL J0941.7+4125¿â×XHÚÁ@Hp}€^_1À;@·E|À<º¢ô§@£Nçï'õ@q<ƒ>?מý0ÂÁ?å
ƒç€­:@È[TŠœ@
eBŠ¿¿ïë"ÌÐþ‹?ïÿì´É È¿æ/ñ)£gy¿êOž£Ä•Ç¿çõ2F¤¿ïü¾â©WþAGNbcuGB6 J0941+4121?ïÚE2†‡f?qyOM£R?mYõéñâ?o ¤.­Æ?PÈù^áB?Ws	rԍ¨?ìü5ÙçΗ?¹¦€K®˜ô?«Ð^âðlè?³"'ƒÐÐ*?¤lC'Þ,¡? )I{¥ç?ítK"à?¤BÀÁg1?¡š&$Š?—¿Pª•Ôä?®¢•çix?-Ë"$X?ìTÃÒ¹\? gcf¿?¶Ä^<‡ã?šª®™úË4?šV
3â^?l¯£¶ˆ?ïªÒ|Ce?†Q}ØO?ƒ\ÅòHÍp?…¿ãU0{K?Né°`mœ?Pc
óðCr?çÁ9S2×ï?Êlåúxà?ÃyEࣳ?Æ:ÐðaÁ*?»©¥!Úh?³ù¡¾Ä0?ì#4—®ªD?¥"ë}õ¡?©"Õb-Ñ?œٓ³?²p'#u?ŸYU$ØN!?ã)Àö!QV?¸P$iÇ?ӗ¯û
†?ºTSJKí?¸UݐÁ
9?«JdR:	'AGN4FGL J0941.9+2724?ï¯CãÀÀ`@HëC,¥À:<éhSÀ<Œ_Æ94Õ@ûˆ÷5=@-'$ZR\?¹ùÛßËhZ?¸r*rD?ø§{‰äð@	É0àóu?í ¶ž¸¿à‡)T ¿å:óṘè¿é£L Â'Ç¿àn—Oß¿é$Læb AGNbll3FGL J0941.6+2727GB6 J0941+2721?ïïΪžœ?R[1šzì»?/ëåv´ü?!fНªˆõ?\e.ÕÃÒæ?QX¶¶¼ñ?ïÓkѤÛ?rBñJê6Ñ?JgÜÍpŸ?Qû°´ÄŠ?s

K"¢	?mþ"—
¸?ï¸_ÈÆ
™?p{ñdõ	?Uy8å÷ƒ–??rAƒÑ?~q́¹b<?o'",a?ïǒ%åun?W1Fl>û?h]C§?M7t4…æ?oîÉņ…?N£Ã.<U?ïÛ#¿†?e·
#⋻?B_öb*î?7þC³^Ò[?p%ïz
*ü?dc>å(CW?ïfÇÕYŽ?3–º©û?`-Ý}…ý?gdéa¡'P?'!atp1š?C5üê¶?ï~õÌÓáG?z;Õ®q¼·?cˆž]šX:?^­
"¾ ?‹`e6ÒA?vŸúñ{?ïVÂé—U?w!‰¨½P?'tљO?oC) ‹?‡Ûx€')P?n6%,g™AGN4FGL J0942.3+2842¿ÇŒöE¦@H<'RT`ªÀ;D€'q^èÀ<È<){úL@ ¿›7©d"?þ,7«gø?ÆViGt‰?‡ºhµåÄ?Å_<¦y{í@Pò‰ø¿ãù`ÃdC¿àÆv;Ƭ¿ãÈßëb¿×:,âMf¿á°@¿ã°>¿ÔýAßAGNbllNVSS J094223+284413?ïèÑdZ?PÌ	j¤D?2'ÉMÒZ?E'æç?dܖƒ¹'H?P‡C¾Wu?ïÔÔø·®¥?nÁ+úh"?AAÐw¹w?H¬kÃôg@?smIÀñ?k§XPNy?ïq.㺜?uAÄJ2§?Xè[.‰=?Uß`µäß?‰†¨Ý °c?sŠ¨Q »®?ïµ@JŒ¯ë?`"&ôBªó?MZIàßw™?1L§	ç?€ÚH±'Ã?`šßü?ïÑÁ"«\ ?d§H%­‡?@'˜Mʓ?.†.dŸQÿ?uêì«ÿ?cÒ	?Ï?ïv[c?‹CØý·/?Qþ·JðlL?[.[ë]»ƒ?©#álÓ?‰ôM3(e>?ï(LFÌån?VÒÀ›Ø?`µ•û‹ÆW?Lƒ¨HGæ?˜ßÄažtƒ?€ñš"\̌?ï5–1Q©?ªÉ	?dy®œþò?R&´,!?œª|Y¨ú?ekKËØøAGN4FGL J0942.3-0800?±í™ÁŸ­@@'1]pŸÀ9—2éaX
À<^6=@e¬|`C@ç¡di6?³m0/Î?Âu'ÿ ±ü@AÁÇ@£$fˆ ¿ÁgncµÜñ¿Õû"¿e=¿áƒ^nË:¿ã@*'zÁg¿åb¼ù2±¿ïúÀZ΂¯AGNbll3FGL J0942.1-0756PMN J0942-0800?ïñ¸.Vï?F¢Ñ\¾§?Fæ–Ö§]?<'¤^Ê?Q©ñåçÏ?<§4õ›œ*?ïÞ3˜o]?l6q½M*?F\îÜ؁?SUŒèÈä/?l5,3o.?f%Ʋ-C˜?ï 4izS>?ƒ'ܧ½t?qlìض[?yP¼âp6m?~y±@°"?yxäM¶?ïÝq'Sê?NÚÞ¶ ˜?E‰ñ½?)7€…Âÿ?m,a1˜?J†ýîf	ç?ïéFõ ²?VÉ_?Sú«Ÿƒý÷?J›ž(äî‰?Ywi¼އ?JùÁÍ×ó?—4ö"?†b¦F÷4?Y†‰+ƒ®?hóôŸØ?"îWºe¼Ô?ƒ'èšÉ€?ï\ˆ9}O?Š\½–+?Aïôý	?ƒ˜3V	?‡œ
oí;?€ÿúpyݸ?ï®8¶fB?hØHÒ¾ë™?Vôï'4?A‹†F`€^?"RTÍ(?g	꜎êAGN4FGL J0942.7-2028¿îUö^Áj@8	WG²JÀ:Ö½A>Ž±À<'›Ø'@¥:=h–A?þ£ð4°áµ?Æx»þsc?¾iAžA/[?ø²'¸#È@ÿŠÏ§G­?ïîá"Úíø¿ÒwØ¿cm¿Ó:4g¾€¿áÄÏ9°%¿ÝÀ¯óx2A¿åÍôIéXAGNbcu1RXS J094237.9-202720?ïËÔTU—·?dUX¯Á®?LRÂ9û,­?@¯o¬aS?v‹}›8	š?a¾ÜÆ«OÃ?ï¡&æÉ£"?|©Ri?\/™{1¿?YY
ʔ§W?"3 Ppók?yRC«»ô?ï'ÂۏæÆ?tüìV(K?]÷$ŒÃǑ?FbÀ#W\?‹d~¿)Ÿ?sÃ-"u?ï_rQÏ?qAëãŒÕ?o̗]Ø4ù?P_
s@²?™~Ë%òr?p}@ÎR#?ïšf#±œ+?v«uZé9N?_1K °¹?W!ï‹#?…€Mº•_?t ­§ž
?ï!{äªg?"Q£SHŠ?j$Úlªó"?pëHÕ[7›?˜‹è,Ùå«?'gaÊ0¡o?ï¹ÓZl?"'~+Ïȝ?ggÀb—?Y­ïòØ®d?šûçsj{Œ?ƒ ƒ1:#?íb&"S½?¾. D?'ˆKÆ®và?iz3Š·w¨?²Æ\TÆ?ŒׯF-AGN4FGL J0943.7+6137?æ -r‡‰@EÑ(9-ŒÀ9ý,ðùÒ¿À<q
À²ã@íúCR@Žm=ðüW?´ÇV2ç‰?Œ.·´è?Õ¿~°Š!@Oš¿ßS?ë]F,4;q¿Ýq¹`‰W­¿éOt.©6¿å¹ôMDVq¿ïÿøãú?íÑØÀ  AGNbcuFIRST J094420.3+613550?ïö
74¹?Q@•ƒIÊô?=Ⱥ6®ƒ?:C=÷ò<`?IH먑›¢?KÏ&±R¤?ï×7&q%?tFW¸ˆ?HFxf]?W ~þHQ÷?q[«z'E?p[<zNa¢?ï="NðÃ?†aÝâì_?w.lPÀtÀ?óMƈ?"™dÎ2hã?|ÛÆÒÇ>—?ï÷måqð?7Œ´¯þ?@Q‹ž¬³Ø?+V&XI²e?C4¼"Å!¿?+›p¹œ?ïïˆLª©?YÔæ"(x*?J×ÉÊ ·ð?Gim°Óú?S"
®µ*´?SceÅt›`?ï"Äñó3$?Â*(êÒ>?UÇ;ò)ç?cÏc3ºÅ?ŒÜ ¬ç¸?Å8y†8E?ï.£ˆ0?ŽÈ×A<WÁ?~{¥Å?ƒÿ†^܊×?"úÿfÝA«?‡Fjë?ïâèäIZ?[P@é¸î"?^1Ardl(?R,h!ª/K?]¢ìæª?L®'b+†AGN4FGL J0944.2+5557¿Ë…»¸Ÿ»"@FûŽ\NµpÀ;q¬O~ÃTÀ<üóæIî@—wȹm?ý–¡G
Ë?ډµ@>3—?äûë~Õp@—ÕÄÃ?ñðtY™#}¿ïýv:ÂÊ?ïÿÄ}îB¿Þ¿EE•6¿ámžÔký¿ï°B¿êfì"¨vAGNbllNVSS J094441+555752?îéfP?ŸÀk¦¨\?Š—w³ôAd?‡íYn¸Õ?•"wftñG?™±ÌЯƒ±?â~Ú¾Ò?Ç<0Có(?ÓÖQð&‡î?Ä0.ív;?¼¯çAuɹ?´€{¨|g?êµü—¦ág?ªRLB«?­7¹Ý_UÌ?ºÉ~´qÿ?»´>S«Vc?¦@õÁø-?å–µ@™?­æªÿW?Ï6•aëFN?®ý)Úñˆ?´áÿ"¥b?' \"?í""Hhhc?±oEŠ?¥§€Pâ	?¥h´-øÞ?¨0;)sW@?§©AœmÞ?Ú&7iE5a?ÌõŒ1"ºî?ÙÈïëéPD?Îèû4Fâ?È!±U¢ô·?½Òæ
Ýۊ?迖Ύ?°ìÒíð6?°³§èGï±? ¨ª%$t ?ħÐÒH•N?­tUXË=ï?àóÐ<	6?¶°Y"9ì?Ó+<HR!?ºñ±H6ûj?Åڄ—6æ?¨‹iè{òAGN4FGL J0945.2+5200?ä1|½sq@G´"ÀÀ:YôNñ՛À<•Ìe÷@»MôU@Üʵ›?ÀÊóÙ¬T?ÁÛÕ~L69?ú˜¸É	Ê@[q¥ß£¿Ôlbñ¼Æ¿äˆ ËQ¢Š¿éx° œB@¿í•Œßvó|¿ïú¡†Íäû?ïðÝî]@MAGNfsrq3FGL J0946.2+5209WISE J094452.09+520233.4?ïóbµy@€?S*þXÛ?C
»Î¾ù9?=µOk™ÊK?OjmfrÁ7?NªyÈð ?ïÑ0ò'"?tÈJb óN?MQ'Ž\Šm?Vúˆ´Ôdo?s½¿Æƒwc?pÆÕ¦âð·?ï™ÄˆõK`?€©HV7œˆ?`rŠ=³x>?cÒGo/*?…r;-hóþ?£G:ºF?ïòþ%??bM'šØ?E†én92Â?.ùœ?ÄIy?P8hLÝ÷?7nw4‹Ü‰?ïào´Ì?i[òMɏ;?`a¿N83?^e"$  {?_ˆì6@?`9ÓDÛ?ïgÿˆ‹Õ6?'ô/÷›UÒ?\í9žn)þ?l¨m±Ü?'1;\-š›?'kp'b"?ïH>—.I-?…SXT›[è?k
Ïù:[¡?kÊ}ÿ¦í?"–ÓS/Û?ƒâÜ25QZ?ïέÁJZ?d¨w€Þ˜?c§`Yąî?Såd« ·+?m«‹üNwä?\Xü™qÊAGN4FGL J0945.5+4635¿è=®ün•@Hf¼b~À;åác\ƪÀ=—^Uö­@!ÏÎ_IÀ?þº©êIµV?ÅŘ•2¿¸9ë‰%ƒ?í–?aê«°@!¼:®Q¸?×A¦=–ä^¿êWvßZn¿Ö·¯™¶¿å®ùèŽÊ3¿ÒS^a_@'?ÍãEµ÷AGNfsrqB3 0942+468?é[>ZŒF(?Õ)'±Nt?^G¾×ªð?€áè~æ?ÊVþ´,Ë?Õh±Þù?ïRÑé8µ¡?"¿‹ï؂?qu¬2,"?x=Ï5¶.ö?'HW´Q=Ñ?Ð)ê²?îÁlÒY?"†(|	¶™?f«~•|"~?s×^Eb1?¢}1L0ã«?'ͽñ9T?ï×³°œ?z«¼]ö»?MGF÷!E8?<·|øÅ{í?µž•©`f?zÝÚ]Ý?êg®§•';?ÉUùž^qÈ?cµµ]2HÇ?oU^‡nü'?ÆnŠªÆñ?É@ôWçXÐ?ܭ•?««±U?P?z\ÄaNe?Š™°"™ž?¤ºLèGò?¨Äñ³¢_?íÔÉÁL?YÜ¥± ?nHƒ*?v¤ÏÖ3'F?°lÀÉcº?œz
"?퍷¿…¢¨?£AtÃè
?nꔠ˜áÃ?fä
:^?²ší\³`õ?£…ó;Ï΅AGN4FGL J0945.7+5759?áYÆDóO@F±3 @|ÈÀ:Âð\À<'*¢jùs@[êæhTR?ýþŽæ¸0^?Ãëv?Úá?Í5³Ö†´å@üŸS @
…ÊúåŽæ¿¹)LÕpµJ¿¼µ,òý8%¿ØR'_js¼¿Ù;}8ºÝ¿épà"&þ¿ßVóé	AGNbll3FGL J0945.9+5756GB6 J0945+5757?ïÝÁB;J?uƒ~@Ìõ¤?_·'o=Ï?[ß½}ï?bc)é[x?qªRµíªÃ?ïؼs}?q·TÖt(	?Fâِ5(4?P³†zæú˜?pÅk¨?m+¢« ?ïjl{ºq½?Š`\¸Çð
?y¨á*'Ó¿?RèûĖy?ˆp‡æë?"é†æ<v?ï«´ñ†7	?]kKÌàÚ?cÍBژVì?DH _ír9?€rØ­à1?XZݹ´*?ï¿5ÈÂYµ?t±z§Y?s^#yd2?o'%y4??j
ð=s2½?a®€ù;?ï'ÎŒ¢?ŠØ…Íæô?^MÏ"?eݶ©¼J?‹ŒTGç™?‡æWœÐÙí?îô'V1Ã?"v@†Õ]?‹ ÷¿';V?Œc»ôáŠ?"Ñó¹[è?†°׆›,?ïë¶pj?zÆGä!}€?vž'ò¤c?`,É@_?–Zøó<_?wë¥8.AGN4FGL J0946.0+4735?âÚEvµF§@HW<ÈóÀ;ŒDÄU/À<ÝêPkR^@ ¯7eœè@ËHZ⤥?ÁY°àÝûÉ¿¸ö·Au@I?ùìÅÛA?óc-+²5r¿î~¸—·¿bø;v´Îe¿ê½¦îí¿ë_:øúRA?Þ]JÿÓ?¿Þ3xgðª"AGNbllRX J0946.0+4735?ì»<"?À4?ÅjZßï?§ƒy«>g?Á›z@9b?¬È¾ŕ¹?º1ÆX‹Ô¬?ï"Ô+÷æ½? <9
EzÊ?}%j‰¿é†?‹,–Z ½?"\ÝãAü?–Ø"ôFÍë?í>ÂMlðC?£o'K›?™K¦ÂX?—ô2Õ?¯KµZR·?ŸŒZÇÿ¢?ïjŸ·?}Úö4gú/?]™½\hŸõ?W–"òäæ(?ÒpyÃ?|³Y>ûµc?íO4ݜ»?¾uRE$ÕÖ?ŸÊ×ATe?¹?'žû¹?«'Fƒ¬Ì?°³¦Ýò¬?î4sQRÐT?­Á^hAè?Š¡c£ØL?¢{¬–üB?¦r#j¯?¢²¤ÙBðÎ?ëíBÐ#[?©¹Ú—c?£çþD?¡Mì%Yë?·ãrÏ­?£Äˆÿš3Û?ídÁ	Âmñ?¢ +0?—,	NÚm?"†{'oC?²§2o"k?¡¼æùêTWAGN4FGL J0946.2+0104¿îúz[!@CH
|ZÄrÀ:¶ßh°ÄÀ<[@dtß@!T)΅‰—?ü‹'™Ù?Ëùwœn¶?¾Ö?;‡?ô›ƒEW"@¤}M]«Ø¿éo»^g"¿ÝÕÿ™'Ú¿ämð‰Ó©¿Û'/'y—q¿¤ûg{¯¿é˜=‹ü£AGNbll3FGL J0946.2+01031RXS J094620.5+010459?ïŒ8&ÚVÆ?R¸FR?S=ÿôÓ5L?GÏ"nãXe?ŠŠ6Jû÷?}srzCÝ?ï' ÌÜŜ?…œP¶¯]?a@öˆ?dÞv'ãWã?‡3ü¶éCx?Ž"Æ1»W?ï7ŽÁ'v?'îa±›¤ÿ?a¥5')Ü?UZmCÃÛ?–Ù–íieÏ?'œ'ÿC
?î`õ[¿Ìè?†Å®
ïç?dU¸!¦º0?QÖ.¯Àž?¨«N¿)æ?†áuä#N»?îв1bp?•`³+ãt?j.[Ó ?a7'Àí?¡QûÁÊÈ?"`*¾î³j?îåųEú? žÓ¢Ð?r˜]"0ÚK?€ä{¤—ø¥?ž¡2:ö)?›þÍ´"¢?íÖ3l­Â	?œs4+àìZ?sDò€—g?o2'ö`?°r0ˆ¯?›j0å4?꯯$gµ¾?¥€©(oð/?{Á-rµò?qáʉËK;?Äc6†#ðö?¥¾ë³éAGN4FGL J0946.6+1016?×=8pÅ÷@E·<³åu:À8†'M!À;ק{¬]@æP4JàN@ÀÐ$p!Ñ?Ÿ|/Ùêö?´Û³@^çßwÊ<@´Çç4×ù?ïо"$哿àð´"†è'¿æ—ºÁÝZ¿çlÏ¡"c¿çµ:uFÔ¿ëëJ ŠAGNfsrq3FGL J0946.5+1017TXS 0943+105?ïïÔ1×#Ï?R¶Bƒ'×?:K–éŽÿ'?.'¼‰=ö?YĶE$a?QXódý·Ò?ïÃðr÷ÌÞ?{0$	;ì?Q?v64éÅ?Xx¢3Ë!?y·é©^F?y`,UÀq5?ïƒÑª³?ˆ#vnõ•¿?d—º°æHf?nºnå?‰åÍÝj•$?†bý'•Þ?ïí>è{²‡?C­µ²ò?L?Ë}+?4/‡!?W:–Ü?:"Z>}§À?ï߬^ùx?mdY(·Å"?>žjƒt!?2_ÆäÞÒ?lÔËm¬ú?l«'˼?ïeôóKUƒ?'¾Ì{ežb?`Ëì0w˜?n!à9ÍÎ?''ävª?Í}'K?ïG ÈCó?"€d-?íð?p—C±z?tç…ÔKŒg?šÑ4Ÿö©5?"UÎmÕ©<?ïÒNμˆ~?aƒNà€h?a¨®ç'?QUß½½4?l	 «í<X?Y¡—0ûwAGN4FGL J0947.1-2541?Ó|ïl{@5Ý~Ë·úÀ9cf´iÿxÀ;Üå`A‰7@Œ•]õ©?üɕà§?°Xù:>?¶w%ü=ÿ@
'¿}Xñ3@
9¨…oÁ?ïò'x=?Пà·õ¥¿Ô¡â=wYÔ¿ÞgÚúâß´¿ÜÕÓ;{׿à 4éì˜AGNbll3FGL J0947.1-25421RXS J094709.2-254056?ïô)†!˜?J™*Ë;j?2tÉÁ¥ØŠ?$#b'™‰g?SÄ«»?HIìiþž?ïÈHŒ>oÛ?€(ñ@?Z½Ákk›?pq¼ªóœ?u,IƒÝgË?u^蹬zm?ïœÑsÇð?yãùà'ZÈ?gª;ËX¾"?q8óžî?ƒ
¼ Á–b?tz"ãHÆ?+ã?{lQ'´õ?xã:Ê©?V̤-{I1?¡BcS–½ã?y"Èì
å?ïë)$o)?bŠ;]œ8ë?Aë·üïÁ?3܉ßaÕ?`kèé³ld?bÃW«?ïY¬Ù‰Á?".\ëÀ?nŠ}ԍ|¨?~	öâ²ü?ùÿY?H¤‹D&?ïlF¿ytƒ?…8'©Ì}Ù?u6]ü1Ùµ?|~7).?ŠS!"*‡?}ô¦žM}?íQÎÓôE?–ˆŠq–B?‡6v™cŠ?nC0'?²J´óÖì?•l?Žù<AGN4FGL J0947.6+2215¿Ðüœü®@HJƒ±ÐÈÀ:ðë€ìújÀ<´¹‰$@µE@ûZ~ї?˾_·¼^?Ðe)O"¢'?ÿý&g@Úp'ÉôU?á΄'Ai?Ðgâ<u§!¿à"Ä"ïï¿ã´zÆo»¿åˆ©©µ¿î•³€ y]AGNbllTXS 0944+225?ïܖ'O$?`j2­,»?RÍì"x´?E¦žÿÂÛ?j^ §¬?YLeœ,•?ïÀ»ç¢;)?vëW¥û÷?UK9þ>5?Y•œxµã?za¹Qô€!?rmÜFÓQ?ï€þA'×N?€H›G<?iÝæ¦ú?kš;L&µ$?‰I/B¢˜?{2ÚÉÀÍî?ïUÈãW?hp¥ÙgÀ§?~xº»i¥?X¾_ÔØ[5?‹QŸµ"?e%;ðj6?ï£ß/ûÆ5?uZ]rb¥<?fs¾i¸Ðs?Y6Æ8?kDqžþ³?qñW)7?ï3½*S¡Ï?'¥6ÍõÖV?hÌü>GÂñ?mCCÁáºW?–n»/ґÄ?Êƒõ­¦?ï+¨0Ïð]?‰0¹Ç½?u¹dˆ"S"?w¯›Ñ?• ¾‰º•?"G¯$óåÍ?îG.íÿ!‰?…X|{£$ã?q°á"³ù?tR5»¦?£T8¬ñ}?ƒs6£&îAGN4FGL J0947.9+1121¿æ­J•@F¸ºÇÀ;n'D:ÂÀ<›@'§@ »;'HnY@¢õ}Åþ|?¢#€ã•;¿¾Ìô9ù ?õò-å˜î@Ó£¬íßA¿ël™ñ®-¥¿æo"‡¹E¿éÍÝ~냿ÕòŒ–›¸¿ÕmË"°¿â=v:ÂÊAGNbllNVSS J094746+112020?ïqÀÐÑOz?ž$³ÿÑ{?P­'›ºÛ?D<±ÏÙç#?Ç{äÿ&?õ9åº?ïªûhŽV?´Hu¨aR?X… 
1ý?`Û¡"Mt?'0qÎ(¶e?~Œ4¦Wǂ?ïD2È8¥?†¤XЫÈ~?Z*"µÐx%?NÀúÍÊâò?•×+à?†i7nY¹€?ÿy¿¬?v
<û>?Jÿ3U¶?;Öm¦?lÌú¥Î?v#íæ8?ïNoà@O¯?"ø¸Á…¤x?`­M¿°Â?WÎKGgÜ?"TÑÉ?"{O{î)?ï±è´£¥?¢j´f¿÷?i€RÝ/ä?ˆodî•j"?™Räç;\?ËàFYß"?îÄ
̾¬?Ö¦•U'.?c™džo×%?`öKkLJû?¢…¨Ü8ÂÃ?a`tY~?íħèøã'?œlàïg®?m®t7®nÈ?fÏiNöý?°íM3=õ?œWþ³h'~AGN4FGL J0948.6-0338¿Ñ;ƒêëø@B!ؾr–öÀ:ò6†¤ÊOÀ<|›U[|(@¤L9µ@R§åŒ·3?ÃéùÃÐϼ¿¨ªWVþêV?áõbLM@~á8>µÈ¿à0(QWáh¿Ùgð>Áܯ¿éÕ2ÌÛæ¿Ûà?:¨rz¿ïÿÙ3ã\[?ï¿xPs¶AGNbcuPMN J0948-0338?ïÙµô@>?f¹¦aΆ?Ròxz‹?IàÐ?lÐÏ©‰›\?cÈý'Ñ?ï¿0U÷ó?'4Þy]'?VôՖ~=ê?cÞp/µFÁ?zªŸ€ÚJ*?{ª
G›?ï`2*}4½?‡PÉÍè }?iº7r#:?hÈ¢Ù]?ÂsÏÒÞ?…½nDˆˆ?ï×è}q4?U×MJ2ï?Mšl,.c±?6xg
õ'{?p¿>J¼²e?RñŽp¶k?ïÁD¥ÃÀ×?y\!OAAû?`X!$	¯?V"¸˜:9?w1œ›.ם?vÊ)²•ó?ïdÔCAPá?'ÿwù?a"t*cÅ?q\>ßTµ?'3	†/¶?ðU\
¿b?î̤R§?"Kmø½&Î?s¶Ú~-…ß?r>œqßò? ¾ßãÍù?'G*9yQ?ïkºCf§?zúëe‹—p?kºSdŠOñ?\[θ­V ?Ž"ÚZi?w¬qµqAGN4FGL J0948.9+0022¿áìCrpŠØ@C[¹pޏÀ7Û:,K¸eÀ;ÅÀ–]¤÷@~jM¦¦ó@Ÿ¬EmÈZ?œX¥f4?Å&J*øQ@$»`Iì³@O­·4¿ÑA¹my*¿äz™ú©¿éšñB¢çÌ¿êÐ3¿J-K¿îÇ·ºã¿ïÿ&¼,k™AGNNLSY13FGL J0948.8+0021PMN J0948+0022?î!"è•Þ­?¯,ª.Ç{›?¥OÌd$ËD?¦™ÁP¥†?'<
!Š÷è?£¾Ab¸Û?í ûla@ü?¹v˾xÚ?¢áÿžb)Œ?²S½
oÂ?£I˜*³?¤^©âé?ëòo.i¨n?®¬áýŽö"?°ßÉmù?£õ[pb??¯z=rw"?§R°Ñq?ïü'??‰Ú«Ð¿?•ˆWG§™?†oAՃÛ?}÷P®ïN?fâüš^?ì)5ÃRÇð?ºw¦À¼Ô?¸Ì¶7X2¦?·»çÿœJ?—¦nÀÝ=N?žr8 "/‰?èÃ#'Sú?̅y
FĤ?¾zÎIÇ?ÆQŸMe ?»ßÔL¯j?»üŒNØU?ëQÇY+¦ˆ?²ßàȑ°•?°¬XΣ?¤‰+¢Æ?´Å§,%ä?®ÇQíi4?í"5ú_Ø?¢ôBaÃL?«¶±Z=R? ՚âÖ?–+އ¼O?†mÜsÖ2ôAGN4FGL J0949.0+4038?Ø-ÆTì)@I'½{ 1ÏÀ:{ôšq/îÀ<âž43@I²dkº@ñ^aµ&¾?º7U½¿"øæ'´?ÐðjÌ&´ @¡ïDÆÙn?ÎòŠ÷jZ<¿ãZK:õ†¿ë&qN õC¿ãâg3B¿ã{.¶Ì°¿áäúÀûÞAGNfsrq3FGL J0948.6+40414C +40.24?ïô…µŒ?lOº‡Ë?/Ï6υ_O?#'³ÀgT?Sõ
¸Ä9þ?l?™¶Ž~?ïਟ¤~-?m}³äkc?=ʽse$q?G`®Š¬õ?kžz^&7?it€=ûØ?ï°åš<ñg?w–rf²Ž?Z›äˆdlÙ?b€×຃?€såŽn©?u"Û+À9J?ïñéáÒå¸?9«ñ䱜?@Àci"üM?%v7'~0?SÌ
œˆ^?4çíÜð͗?ïñ÷wµ?W.Ob*¤ê?:QLõâø?0T¼VM?WA±<M]?U¨»ä/ß~?ï"÷ràÉ?ŠœÛ«?Pd)ñŒ?Z©"?ôKg?ˆ¾V¹ágØ?‰Èâé£?ïvKQî¤?'È	uóo?bóî×;:?i.hiÌÓ?°<v½qq?€ŠÕ¡Þ;?ïÓ0\ÐKÄ?ZáãÃ?\ûˍ G?G¿ˆŽRíN?nQ½ƒIô/?U'"•ß&AGN4FGL J0949.2+1749¿Ø/&úüÇ"@G'«!ZÀ:Â㨱d'À<ˆ–&G'f@<ÁQnˆ@öå¥
ç?Å.Bž
A¢?Œ$P
Öϧ?ÂèyfkK@ø÷2Q
¿ì]ÒC.S¿¸¯ƒ»¶Ð¿è¸5›Ã?…¿àó›}Ê[-¿ìE¶ù%ñ+¿ïÿÉ–oAGNfsrq1FGL J0949.8+1757TXS 0946+181?ï때¤~?V«ðûRŒ?BKb ?2¼_Zúóg?_¯!:Bž?TLgºø?ïâöm?mø@¼³M?=í®ŸAã-?IJæARÌ?j;TÍؙ?i?²ˆÂ?éZ€?€Ñg° @S?ij‡{ëy?sHl®¨³?…€ÚjvÎ?{¯bOÄ?ïìWƒÁã\?A·Æ8Z?Boô£÷Ä>?%()úƒI
?^þ®Z'??h—n–`Í?ïÜý( Ì?fº&€Ã?Lò–,¨åz?CÞgܔg?kÆ1â*
?cL>ÉF·?ï™·½'?‹¥=#½m‹?P˜w>}¥?ZbšÇãv?‡µßó®Û?ŠqNFÀöÙ?ïWK‡«'?…TÈ ™Y?iÍÁ'ÿ›?n²à•<?'Üæ՟tÉ?ƒA§5R¹?ïÌÓ^Ñ
Ž?`±£<Ñ/?W§M7q€~?DyT!?s¬}M
ôè?\*í_+™AGN4FGL J0949.7+5819¿Æùy—àJÈ@FÝ]Ý*èâÀ:=çi0EBÀ<x5k×Í@Q¡?*bT@Î=EìÏ?º"tôô‰)?¶ûOþ+OË?ørÀF¬Œ»@zùdZr'?ÜÀÄÖ´,¿ãG(é-U¤¿çkÄߘl¿ë[î¾96-¿Þ¿â®‹n¿ïû›ûs©AGNbcu87GB 094609.3+583301?ï÷q³møx?B8ByüDÂ?*ÑC­®Ü¶?YÑ3ö¤?K"â[;Ü?@w»sï?ïÜfüÊ|¢?pêf¨ºü?B¨´S
½˜?K{Å÷>Ρ?nîÖI'±%?kÕ·bÒ¸?ï¼'¾_÷Œ?q
Ó-‰-?YÒ_8ºµ?cl×_Å?{w‰×?k¡¤x¬?ïã
W›6A?IÃxÅ]ã?Q¢É93™0?7"X鱬ä?d!C˜k
?F3-9þL?ïï=Ú£q?S=kNºC¤?7Óõ?r?/…ÒãuYk?[M¢äˆ¹?Q+ç{ƒá?ï'Å«#}?†  ÙTʧ?Rø8FQ¢Ò?\\2²Ø?‰/Ž6YÆT?"KU*_==?O\Î?|qíe™÷?c18þ»=?edVŸSU?‰G
à²?ª?x×Áà&í?ïœNvŸ]m?n7µ"Ⱦ?oÈ¥–j´?]™fGXt?€ú8ñ.E)?i( Õím»AGN4FGL J0950.2+0615¿à£Fñœ@EFA,ðúÀ:Zˆàä±ÆÀ<n;è
šó@ÐÉéC?ÿ`_¼(:?Á ¥¼è~.?ÀØÉÛ*Þ{@9}I׺g@«ÕÄF™¿ïÈ͙{f©?ïÿ3¶>ì¿â¢çUåã¿Þs²LîÆ¿áG§~´ì¿ïûÇVkF AGNbllGB6 J0950+0615?ïÞ]ìn;?m6µ"¨øº?T¼ð'|Ñ?i=tû÷%?gC›¥S\W?Vvè§l{?ïÉHwVè?xÕëC*X5?T'
Z.?^º>è?vUÙ7àv?rŒD<âß?ï—jh1JX?uû	š4S'?ci`òÙ-Þ?mõXÒÂ?…K
ÁõÞ]?plY½/#Æ?ï!íP%u?oÒ<=ì÷D?'þ¦G€?`ƱÚWm?'µÓKž?hMÂÐ>?ï¸ã<a€?'êGÈEÈo?q.Ï©$–Ø?'ß—y¤?r_')ÀE8?_)@ÎÙü?ïUù°î?'æYÅßá?huM ҂ù?põ"e«í?'2 Wœ¿?Ž;jJ‡ÉÊ?ïFŸÆJ?'ªpK€~?l¶o>1?mN}¨Ø"í?"•9Z0­?~ÖÎ3üE.?íÿ"fù֓?‰w3²å‹?"Lîy¾à?wËJ8)ßo?¦a­šžf?"fÍz­×OAGN4FGL J0950.2+4553¿ïÒ*òiP@Hß`|A™þÀ:¸7êRÀ<…Q(ÀB@ŸTÄ}s?ÿz"¯tÍ1?¶-z¢§>?¯6¨¢e?ؓÓ›fù@<ȋ­?ê;KÀ¿n¿ÑÄÝÀ$5¿å4Ô#&¿Ò¶´DÁ¿â2«ž~Û¨¿áÊFà!AGNbll3FGL J0950.1+4554RX J0950.2+4553?ïÐWaÌßÓ?bô»@è?RŸ;w­ê?@(™­N:c?s,€/õïæ?_]Ð|šq?ïϏï:¤°?ua'ž9>?N˜6HO<?VñØº{š?te"©Aº?púI¼?ï|ÀþZ9?yüx£€|?aæ»ÁŸÜ?U'¼"¬™?ŒVLªâóÿ?xwm+õÏÂ?ïiÀݗJ?iX·ûÿJ?y†Ã'GQ?W¤	"¶X}?ˆÌ˜N´Ñ«?cçÍ^a?כּ‰ÐÆ#?p'‰ÆB
#?`ifÀ?RéYÙcÖ¹?€¶Ã×øÓP?l'¹'†[?ïPgÿ÷$B?¡:íλi—?`)ZíŽo¹?h¥ŠƒM?"íԟÎÒ? ó"¥­±Ñ?ïIäê>¼?…Äüfûª?q†Ð-UÑ?q0|ªŒR?š•Y)àü?ƒ"P…O?îf0•Áj:?‡7•ø³?''a¢úo?u}·¸«ê? Ü-sóÆ ?'K¾¡é,ÕAGN4FGL J0952.1+3932?ì–Çùd–"@I€Ž6FÀ;rð\À<Ø£oqY@!‰Œ{ÎØk?÷êÐ"¢§?Óå¿âÙ~Œ?ÌyÞýPù?ü5K÷OWV?ô ˆ­Ž¿ïÿÿ" 5•?ï÷‹Pb?í€ðÀÇÛ̿ӊi%¡_¿ÔÌåÄ—¿Ýx(Z½ëAGNbll1FGL J0952.2+3926RX J0952.2+3936?î-!^¨	§?³¼›C(Mñ?bü®nq&?hµ	«à!?«þ+ôw?³žŽ9Ø؎?Äã|ð?ˆ
÷žÀF˜?gó¥ß%"?s×hnjÍ?"á%Qüª"?€örçîÜ*?í¹dN¢ê? "ù"—4?ƒ®)­?‡²†VŽ?¯~0ÒBÈ÷?ž®¬R
Pç?îµëΉ?Ž	ÕÃuÈõ?†°õ1Ä?s²›åûz;?ª-u	:"?ŠnIè4?퐜3Á'K?´*µzꏨ?k¬ gæT?i~lk/ó<?²½aª&ö?³ï;…¾Ðž?î¹ß)›¯É?§¿wŠâ-?€Ú	Ž°š°?–šÒ{MÙF? +‹f¨<? ¹yù_4À?ì¡{M(QÙ?¤/«AÌN?Œrý¸!ûð?ŒÙZ¹Yß?·eÅÞÝJ½?£@6–êé?ìAcƒnE>?¢ÿ°?ˆ¨<Ù±)?'
;2Õ'?ºßáý`"i?¡£+Âë;gAGN4FGL J0952.2+7503¿àãÒhJʲ@BŽÌ¼Õ,À;}§´æÀ<÷;«§¹@#2Xëÿm?ò:¦ú«,i?ÜHñáYKÌ?Ô¶VÿIh@¤m'Lž@7mŒöH?ïOÄÞì´õ¿á¶2 ä|¿ï¡±`_¼(?î»4ßZÃñ¿ª]{íñ¿Ì‡Ú¿Ô–ÆAGNbllRBS 0804?9æ?'š)§G¡?ZïàÜ!÷?QqÙ"Nì?‰r5žê³µ?çÊ{ý
?ï¯3 Û3?‡ÎVðDF?[¶Ùú3=?isêj!?€¼<'jÈä?"#@Œ6(Œ?î•qÛ~Z=?–¨lM0a?j¾òƒ:"—?mþþžÑ?¤üó ™ø?–&]{ŸøG?ï~Gà#Û?|³EÆj~?L뿙vӋ?M>ù­
Ûr?ŽŸdï©°?|c¡2$u?ïv<Oð
ó?‡¸‡Ҋø?gøä7Œ†?a`ºC1?Œ«íÔæ>?†W‹ÿ"x·?ïDÿ´‰<³?œ}i`(Ð?f"œ-ä?|µf‹p¨1?"›Éã*ð?˜üöúâxŸ?îã4uÜ?šëŠWPV¬?qWo?s­š=g™^?­'Iتë??š>,1d?î+'eô!? bj‰YÝ ?lxË´š	?x1]E/?«…"SÔ?Ÿÿ§n6óAGN4FGL J0952.6-5048?ïõTEÛ	.@9¡vݬïÀ:ªî!±*°À<2kÛñ,þ@ rUãâ=!?ÿD*Lä'?ÎۂGB‰½?ËÁЈgB?ýIƒ×u.@	qÁpÎ\¿ï'Óa'jv?ïøx·¡Â]¿ÔìKî¿ØCe'Š,¿éý7%?¿È¡ð•©ÊêAGNbcuPMN J0952-5049?ïKyB·	Â?–˜2fY¦?f`çta‡u?c"ê£J?"ĺ±K¤à?ŒDE{˂"?íCv&ÍÊ#?¶S2Ey;=?bZâÝ®ê?q	N³™Vr?µQw±d›?µ¾]Xï²?íäƒÏF¾o?›«|g|…?Ù»J~á?>ZS<£Ù?­Å§Ó8ä²?™ï¸ˆgÛ?ï}•_«À?s¾ŒV0×m?pý<Ñ¡ƒ­?QàȃB9h?˜pþ%ýn?r°y?î)gçè(•?¤`Íúc!Ò?|.]ï˶?uÍå—Ç?©ãµÄT?¢ÿsÁî¢?é|UºWæW?Ã,åç%?|c\&4²»?•iik¢'?É+Ž6—ŸL?Âþ·¸¤³?ë}Y&âÂØ?¦>eˆž^J?‹ƒë¨MÅ?"vøteÈ?ÀR\¨;aÅ?¥M«žBº?íσÚPÕ?TDa(<?€£à'pj?jʤö ?®ÞÊ9`Å?Ž2 %{1AGN4FGL J0952.8+0712¿íÖÒ(p%q@E£?á—_-À:ñùÌàÀ<¢Jmâ[ª@ IúõÕ?þHåL"C?Ê¿Yòª?Ïã}h`'@]ˆ~¿"À@Ën–™	¿ìø0Èõ§·?ïõ>¦-ü"¿Ø"GNNí¿ÔžÒn¥Ð¿ïþa?ïæf¿QºAGNbll3FGL J0952.8+0711SDSS J095249.57+071329.9?ïl÷v]n4?'a'¦ãÚ?'p[¶s?Šðï4ä_Ò?'R
¬oÝ?ƒ
"MÉÀ¶?îö"þEÚo?ÓÁ_¤?†1ÎHÔ¨?'–Ð=NýÛ?–yc±Ó?Ž¨ÈLÀE?î7u^j³A?˜rzšµó?'n
7ü?ŒçßÞރj?£Qœ'¸Íé?"G§Ú0*?îVöÓ ?j?‡1Mër?•1´YÄ?yŸÌÚ}Ö@? 
ˆ°'x{?€ sK|Ú4?î"&¬ÖÑø?'"w(›ú?œÕûtª÷»?™?¶I3ÂÔ?¥.雑K?ˆŒHrÀ?íXlya&?³ ,O9/>?š~@…}Ä+?§F ®rÚî?­:%vî/?¦35z?ì¸{JèËJ?¢™Væ‡,0?äxF*	S?"¿üE:­?²Ã˜
[?ž€1*ÔÆÀ?ëtg¾Þ«$?¡U"zzNä?©¹¡Ö6Õk?"¡ qp¢Ù?·ñÉz¬?›ë©Ä¥…AGN4FGL J0953.0-0840?ڡتß@@óO?Ù3ãÀ8d.˜™¿YÀ;n­£;ÙË@ßn"³*å?üכ'˜™?£Ú!þNò?§Ë
te@ždoa'@
v4‹¢àë¿ÊæW¸M¹Ç¿Ü{±|9av¿Úä1ò¿Üžt?¿Û#'K¯¿ãO"þ)f+AGNbll3FGL J0953.0-0839PMN J0953-0840?ïìu鳄Ê?VbëN[B?(êCt	ù?õ÷'ÅòÀ?aûu
Bb?UŒš¶"ËÔ?ïÐÆTôµ/?r‹®^H?JÌPºË˜;?QñÍBj•?tCKÖŅ?p;Ê¡Cp?ï§UWÜq?'ÿI•V?XÎfùˆëj?`²P'a`?ƒÝñ.?}aÁêV3?ïHå(°š´?xÚ\ïMŒò?`LM–äd?Aš™ñÝK?"ÙÑ=Þ?x$¥•=!?ïÊ©{þ˜?pˆ<?B€??;bFµ¨?5Cåc@Éù?y	u:çÌö?nâxŠÊ+¯?ïp:Çý?ŠIÖCK¸?]¦†óì϶?eÔtŸÛÆC?%0;1.v?ˆ®;ؗ?uÚ͖?†C»D"êr?aîÒ>ÿTÁ?pç_Äçs?†â.	²ï?"©fB ÿ?î l®ÌS"?ëJÉúJä?kly%ò-?U
ý€½m?¤Bm"Z½?´ñ
…NAGN4FGL J0953.4-7659¿Ô©+|xUÀ1Š©Å`ÇÁÀ:½c€ßÀ<`wç˜*.@ ø£8bG?þ¯(¬ÇsÇ?ÎÙh¼ûî?¡·×GO÷?Ñí_‹Íÿ?üY˜Ý±÷^?îz	{©ÄŠ¿æ³"µ!¿ãÞÞyÈn¿É@٘b7¿ãûD^Ô¡­¿ÇZ<!~|AGNbcu3FGL J0953.1-7657cRX J0953.1-7657?ï»ípø?n(²›-a?6©wÂgù€?&¥Ü;Hu?€Ot.Ž·?m…ìèoñM?ïV÷‰?ŠuTÞ<;?ad>*ÇM?gþvA=¡?‡à÷§ø?ˆÎÚ¾Þêµ?ïfKÔÈLh?x.S¸}Ú?_Uþ:Nâ?HÕÛgÏ?'A%z"
?w,¶
5ý!?í×3Éí/ª?…5²¿Zsi?xb¼Ä;û?Zt9¡V
?¯€kÅ&äf?"í|3e(?ïwÍç~ÿº?€KÄröÄ?D"!N^?7ìjjù?e2¿D|?ðýÓ݇?îæªn~ö? úƾÂ}P?k÷LE/Œn?xú;Ÿº?Ÿ«Èž©s¸? Ll=‹"×?î±/y";?'i	¹$>ó?i¸ÛÿÑ?`ˆ«¾<ï¨?£\ŒÛ¶˜°?Æ%â¿\µ?éΞUr'?¡Qý9+c¿?‹RE]‡?yóù.¦?Çuänæ#?¡¼´"AGN4FGL J0954.2+4913¿Û7€ÓW´@Hɛ^•·À:¸®.|NÀ<iU1Š¼‡@!¼'?ò"EW"%Å?Ë*D¢s?ÔÍ¿Ü#å@
)
]Qï?þ%2êc
¼¿ïêzAå}ž?ïý³^f¾¿ÙÊɝ}u?ÒóbÎ+qž¿ÛV¿\W¿ÐtéæAGNbll3FGL J0954.2+49131ES 0950+495?îèÉ^òî?"S©™m¯?…ˆ¬¦*f?|294g?˜8ЂÄ'þ?·8ôÊ¾?ï‰A=¼?ŒÍ,%õHq?o+w|·þ?y·5®/J?…äÒõRIp?'ãò™=:â?í!bä"W?£)¬Ó†p? ªÊëâkä?•è:¹?­?Èh†t?,ï£ñŸ0?ìNic,0q?œ.kh?'QѼ@?|z</#å©?¹8@u¿^u?šÃŸ†Öcó?î™ËÀç?šïÉbž¬?…|¥+Ãß0?

T0j?œît%ó‹?•­®,Rã?îUTáŒU?«²$µcq?ŒÉ °TÀ"?›‰">6É?£xI¼ÝL"?¢ï+@|p4?ëQyl¨tÔ?ªë¥È)Ž•?©'Ü£5wý?žR=êË5?¸²ÆJÙka?¤•%§É?è‰ëm:¯Ã?²…ş_?^ÿkÙ?"0Á@ñÅ?Ê4ÆjKçú?²¹·ÏÃ)éAGN4FGL J0954.2-2520¿ääMÕJõ@6_Až0PÀ:¢Iøq–EÀ<~ÑF¯ú@ /
Å"?ÿ‡šÉD'?ÄqÁ¹H`—?˜Žd.d?ØÁ—¯@÷
ú¯ß?ïÿ!ڛB¿Ür½'ÈF¿çp4摙ñ¿ÄP'à™³E¿áHÍcˁs¿ä'gÁZRÝAGNbcu2MASS J09541965-2519588?ï¸gYÍÉ?pý1Gao²?H!ÇT"EÈ?5¨¹‰Ù)?€d
"TÍ
?pt"š]ç?ï³Ì(?~5¹™ˆ˜?ULÎþúÂ?[V >V.?€óû½?zŒåÆ㽡?ï@i:•?†RߧÄ?dqnœ³±ö?`'"öNÏ:?•d±NyÝ'?…ríÇéð?ï0SÚȍù?q8À[:fk?q¼Ð™u³g?Q_Âh?•†Py…¡?pif¥kSõ?ïzH$JÑÏ?'†,)֟~?R¸‹ÈWÁ?D L%6@?ô1+?'üÒ؎O?ïO¿êLu¶?SRlÇD?_Õ$"K®?pDzI?"
°gyQt?X¾™>'?îxH9ÖŽ?•eåe‰—z?o¤o.Ãr?fˆ¹b«?¦5rô+p?"Çì1NÔ?ížÁŒ&êP?Œ$Êî-ù?‰š9+ä˜?qWKz?¯­Xót?‹(ÄÑH
AGN4FGL J0955.1+3551?ïüãŽbâV@Iß°_®¼AÀ; ˆÂ±ÀØÀ<ôæ¾æZ=@ œ"†Z"?þ$àŠó?ȦˆÂÔ?™µ÷ü®ðL?Ô|Š_iòã?ü¼xÁ²½?ïüÿ?:Óf?Òß<ã[/¿à¢»ìª¸¦¿à. ÿÿÕ
¿áÃ_eÁ$ù¿×m\D#›fAGNbll1RXS J095508.2+355054?﷑­£"?~ü°´N`?Eá€ÒàDÁ?O–ô¨iG³?€½|‡˜ð¼?|­ö7Ê/°?}'u?"Ô	…#'?aÃS§öíE?iJ­HÞ H?‡_˪~gf?€ˆ#ÐÁ°X?ï"¨®àR¼?ˆã†t9=?påöÁRb?tÁp…žš?—qlocü?†Q°ü֍'?ï=5ãð2‹?tñ¦¸ö]?{'¤»iU¸?aˆ<fn8?'tšL@!8?sBwY¥Ë?ïp©¾ÞU?'²þCŽ
?PWŠÖnÛí?T&
4¸Å·?†˜ä=ç\?'Ü_áð?îþ°'ᬔ?šPZsY?l
ÆYƐã?rBseÒì?œ¨B3>6k?˜^ï%q'?îw·Î|¿?"]±XÊi?xóïÉœê?yð.5l?¥fv-q?'ÜY$
z?íÜk,Lÿ?'8V2¼•È?~§+ѵ­?}@Duq7x?ªY¥qjÛ©?ë'n­*€AGN4FGL J0955.2+0835¿äÑÔX²H½@F=ã!¢ç÷À;Fiž)KSÀ<™§ågÎ@D‡Åܙ@ø¢×/ý?Õ@'&5t?³Ä»[`Mó?Û£VœCíì@4§®/RÔ¿ç=:¾Aê|+"Ù@y¿ç0iTWp)¿Ò¦^äfòR¿æuÌ}ɯ¿ïò›]¾÷øAGNbllNVSS J095501+083342?ïØç$jT?b^¨<)½ó??æÂý'E?.µhÒ5Õ?qŽµâ¥|?a•ÖLBšÐ?ïÁ…Žþ=¼?"bsjkeÍ?JpÛw'-l?O‹î†õ˦?{ïþŸtþ?ƒû{óÿî?ïlØ&Xj‹?y£•>Áú?bcbª
°?c(¥Q½?ŽÖÂÐè?w_ד"²Ý?ï p3ªã?aÿ9mH?SUU?1t?7>,ƒû¹
?…yH|Áó?a;fPsO?sk\š?|˜´½ÇJ?LÐLŸDE?A#r¾å?‡ÏÞ[1ØT?{úÀ®?ïGr;S5?"Œ†'û0]?]Šgm'™Á?eÈ4±ok?•5«@\§Ñ?"ÎnñÐ?îÑÀ‹I†?4qéÕ°Ç?m†MYø‹l?hæõ×*ôH?¡š4kŽç?Žl†òë?îãªi '—?"tAN¶'À?d•è†§ÿ'?U;ö´Ã¨? {úÛՈ›?ƒ¹Fi•ÇAGN4FGL J0956.0+3936?îÿÿƎ0@IÞ<âž4À:ñù²%hÀ<½>Õ'å@`ÕwuW@Ò7y…?Å
½]Äu?ªéLŠGA2?á…Ñqw<?ý"È<V?î™Ä%^¿Ö‹_ú¼t:¿èŸœb¡µÈ¿ãV:Ÿ8?¿áBUå墇¿ïÿú Âî'AGNfsrqWISE J095608.57+393515.8? ,Æ?˜à¬`m>?V‰ép:?UE=o¡Ìb?""†ãži?˜ý˜vÍÊ?ï£Ãb(?w|O7ú'?]0u̵?^Ãì_?ƒ–K[ËP?t-Ðœs¢?ï5^ò‡O?"åžuZ?ye‹=_®?},m»%…?'úÚÌö°y?e"£ b?ï]ªÏ»=?p_Ï#aT"?'œ÷H֛s?dº&‰ô?…øTϊù5?dЏI;Œ¹?ïŒyDø?ƒGë&*?[úÐ!]KI?Q'Áê㼒?‰z»²´x?'DÐLÁâ?îàˆfˆ¨?™ 1ãLÌÿ?r¾²"O W?x
pŽWûû?Ÿ?F•OWã?–¬dN=›?î 1üQt½?ïŠ…?'ãvõdL"?‰Þx4[à?¡Dzø—?‰Z-p‰R?î/-Kw~?‰¾R̅É?™á
úãi$?ƒƒ+˜? ¥Í
ˆ?•VM~AGN4FGL J0956.5-0958¿ï«.y5@@ÖÌ¢Ûa»À;‡þzÄÂ<À<¿Ã€ó°f@!ªpI¿Í?õ^x%«‹4?ÞH×à&?Ød¡ŸøXl?úª(Èv%÷@Æ+rõk¿ïúŒ"¸'¬?ïÙû¿(Ÿ[¿çã4å2t¿½‡âž+ŠÙ¿ÜNczΨD¿È§^hÁ	 AGNbll1RXS J095627.2-095720?ïÒ±Vqù?k²ÞM¡?Kç¨9?G6""@?s*s~ÏTA?g伯@?﹞@ê£D?'úÂI(?T·…2×0?_Ü¥•Ü?~ûl!XA?|õË5(o?ï¡h‰Æ?ŽÉ(؅J?yó.·«®ì?€Z`lÓó?–o=Ä®1?‰×y?îÿœô©ý?{€ýŒwc	?`á;Õ`y?P ˆ{'Ë?ð:f5Q?zæU½Z‡?ïƐ)Xi?p\¹!×?Q'€ùé©:?Güÿ!È?x'—­‰M5?mýÎH_,?ï=ÖÁ²]?™ö…ÌÀà?i¿wFÙéK?{'Îh<Ü(?•
8çkù<?• £˜ÞÏ'?î"8ßox?""ÒNCê?{›7A¯~?'Q²{›?£Yîž?'ŒÝò»©?ífõ¤U?–·4›N`Ç?h¨¤)º–n?fm
1‡Z©?´
65©?–râV¿óAGN4FGL J0956.7+2516¿ÓÖцM•@IzÒ4ëšÀ9FÁ*ØßÀ<Fx*´±@zŸÉ3%@ç	#•0~?­PLž"*?¸cÐ^ý'f@~5Å´ª—@0ïŒv¿Ðû"‰µ ¿ä¤
ájÿçb)Àê¿èû¶ßû}º¿í¼{Eñ¿ïúàSG%AGNfsrq3FGL J0956.6+2515OK 290?ïðèy6ÞË?LööEd?>' ‹¸¦ž?0A,~²?V¥%..ÜÍ?H½èAäDe?ï©x=y«?ƒÙyn,Â?_c
æÒmZ?jôÏϦeï?µ}é }Á?1DL‰f3?ï¸s"+N?u|ŽìÄ?_°¦v?`SoǘÅ[?|t"ol?qD¡h¥g?ïÔåX—‹?T«ší"&?hÀÌp~ì?NÙ3æ-¢à?cç<þG?FÉ'> Â?ïàú)‡
?d8-ÇM+ä?I†Òµ®s?;àÒȚrZ?hڑ†"·ò?b¨IqûP\?ïSj'¢)? ü´ïÓ?k'WÜR?}…*Ü(‰?™Crgóі?ŸÎM 1]L?ï|¯zÎÊ ?'/%fÔ»Ó?dãO§$u?WڂÇúj?‹Óè€ú"Æ?-õÞ>8?ÐÔvî?x\_s h?'Q@á…å1?pê_Vh¼?z€á'¡?gä\ŠiUÒAGN4FGL J0957.3-1348?ïq¨ºÚî	@?.+{®ÍÀ9¦©ÑAåÀ<*ø; ‡@SŽºB†@zÕٻș?¶r ®Ì1?Ãà:±@0
ÚN•@úÓ>«âG¿Ëƒw™?¿á†"S¼ì¿äŽ4 C€¿èqéòwA¿í$ŒVºø¿ï髕D CAGNfsrq3FGL J0957.5-1351PMN J0957-1350?ïÑü:èM ?h;7Þó{Ç?aÙ÷r7?[$•dlmg?l*¯é(®c?^8»K«º?ïØ§V?piÉàšÈ?J;ïdò
Ò?XËÌ'n˜5?pA?½fœ§?igSn
£^?ï…õ»Ÿí?ƒBµ«ù»"?w{ҟ¤¿u?{+^˜³µæ?'ħôUã?wãŸÙmÿÁ?ïâBÀCý[?K¼=bSÂ?R¨¯Nûa?7õŒøÒwÀ?dhè#ýϑ?Cʇ߈í?ï¬ &^?p£è,¾?hËá??_EܶUcH?rŒ²¥¦?g^Üj⿃?ïv«U?ˆ€ê©?ar¿ü^ÿ£?pùŠ¯–½?‡Å¯"[*ï?"]"M·_?ïÄú׈N?×—#®F?ˆm¹ Zƒþ?ˆÍ,†*Wì?'ЄQPB?"pµÜ…¦l?ï¸åkÌy7?eöº54?e²¶~µEO?Ru%r¦?x³îê6õŸ?`Ûä#¡áåAGN4FGL J0957.6+5523?¬‡Yk¥AM@G÷7âÅ\–À7Ìo¯»DÀ;+Šƒ|!@º	^" ?þgbzH›z?ŠñnÝ`÷?´
š7Ï$@@%Áã†Lµ»@
%@톿±ªà=íÌL¿ØběOý¿à•OB2"¿à[
bY'l¿äS¡2OB¿åTWp)]ÇAGNfsrq3FGL J0957.6+55234C +55.17?ïm÷Q'1j?;ZÈC=Q?p˜:Ù7Ç?|5¸>buÈ?Œ6Ÿþ7©?…ÜËè¡??âþåi.ug?×q¬äÐB?Õ/à%w¼X?Ö
ñÍ.¾Ò?³IT!‰Ji?³ã¶\Ð?êÕ?/c?±¹è–^4?º‰ZB|ãg?©2~f1.?µOûÃ×Ç?¦¼"€g×?ÝÛÀ'fU†?¶×l'Zí?Չjk¸5?´ú_ö€g~?É5ªº[ä‹?ª—8Û?ï6>ÀÚü?˜8~R¦_?vVÕh–†.?x¦Eø?"¢r'5ûy?"V­0±@?Ú >	·"?؆'祖'?ބO¨BC?Øù!'I?»mˊ'zn?¼FC'¿Y?ê#}Y᷄?±0ßFd!ï?´}¤m•?§¡¦ç 2?ºT—‹;KÊ?¦ú˜IþÊÍ?ÒëyÈ÷^?¶çÇ*õ—´?ÚG:ùÈzÐ?½Hä½.t?ÒͶŒnÒ?·ú*Í6"MIXED4FGL J0957.8+3423¿ç»£…¼Ô@J&îcŠ	À:t¥×ÛÀ<®!õô
ƒ@)ÒÉ*@q<%J<d?À–%›Åî·?ĸØú¹>@(C(†@Ž e¨"?ïû›¢|K¿ÜqÎäÕO¿ábTŽ†@¿âWÝ6§[ú¿ç¾RúÉ¿ïöCôK–×AGNbcuB2 0954+34?ïïSE³y¦?T÷<Äç?P&);O]6?LG«'›úÄ?Q3K…ß-p?Dx»¤ú\B?ïÎbxò°?u×Ã[ß>?Q?2A/?Yï½5'Ƙ?t'Ú?pš"‡½†?ïµÍpü?l"uoz*£?_µ•P³?`9åºf',?},ÈñÓ?g_sÀ-p?9s$?bmý…B?t¤"Žg7Ð?Q0i£¶j?…PÒÏqø?^<C#"Å?ïÝ÷ŸY™?b0÷ÉĒh?d‡9áËQ?]&?Ë@1~?[Šõw?NXxÊr?ï[_~X?'"H'-u?au
ƒÖ«?gó28u¶?'ezV}þ?­l·]s?ï}'ɳ?}6ÿºd?pnñúו´?qï³À+¹?ˆd°ê?u)××½Y?îَ'2$É?€ŒµŸMS?‹"º;ãw?kî%¥ Z?—Kãã|­?zþð]#AGN4FGL J0958.0+4728?íþÉLmI@IU·|¯ÞÀ9›"²ÈÀ<1Ø2[@¿B4Íg@ì&ÿ½?²SõuuÊ?Ð?½t•@ge47?1@ùnõG¤?Ìÿ‡	I)ë¿Þ²…³¹€¿éTÀ¡›EÁ¿ç‡»JÄIq¿îíŒàΌk¿ïÿ "_õAGNfsrq3FGL J0957.4+4728OK 492?ïÑPü-?"œ)Ñw?–³8á«s?…'`…ë?€¥;'»#¹?òý{$ëE?ïÂw\­Ö?€âè+pÆ»?T¦ª˜,G?bw¢•Âþ?yÐÁpÅß?}ò&¢ÖE?íƒo§
y?£ãÞGª?©±¯`¼iŽ? q"Wé×?œ.¬[€=Ú?"ÁªŒ?ïãʕÃ~Î?Ms…±£Ý0?ZCYe.?CCŸ€#&ý?^'¿Ò]ng?Ap€57vç?îOtž–?¦Ï°»uì©?§æ«2hö?¢V@ú'@9?
œ¿)P?'Ì3P¸ŸÜ?ïL=¹°!?šžUä¦?m¾Á[©mÓ?'ÙŒxÉÀS?'Ä€Õn8?'KܖQ7A?ì/1ñ¿ i?ªøªåá	´?±F²Ƹ?£†ST†'?ª|Ãè%-? ƒÁ6éÖ?ï¬+¶«çê?oÌ
(ïLÓ?t0¦ûÔº"?cŒi™šp?u¹}¾µp"?bÅÔ»y­\AGN4FGL J0958.0-0319¿ïOÛÎ%@C%? §?À;œ¥ŸaY·À<Ê]Óð­}@"˜ÕV‰#«?à•<<Ç0¬?ï6jXŠÜ?é±e¾àÆ?üõÅêZ|@²Òû¿ïýcm¢?eÆ-¿ÖUGZ1¥¿í€ãŸø†?ê·ãÑ̿⨈ŸÌ8¨AGNbll3FGL J0958.3-03181RXS J095806.4-031729?ï¿Â'ú?žFùïÕ?€¬Í.ð¤?šYÎIñÞ?–™¡iV6Â?'²ºal*?ïb.7Ã2<? "L¹Ÿ§?l÷«YGâr?}ÿ†¹G?C¤ÛÇ0?œ0šOí–+?í®Y¬†? Q²h1<š?•éžyQ?'Û²¡[
?ª%ê0y?œ~	Ãï%?îBìtîü?–¦ã"]8?'E9•;U?1™Ák•ª?§ÔŒ'2Ï?–£
n‰n«?îŽ ,xâs?£ó^ˆ«É?'û3>¨%³?'ŸÞCK?¢_0i¹³ê?¡Œê'\Gú?înïs.º—?±ü§¡hFÆ?
¼ð ô?"5¥®nÌ?¥/Q+Š«?¯2E£Rsù?쓨_ÉØë?¥³¥õ¢¢å?š¤h¬F,{?"…$œï?´¹¢×éˆ?£2g¦rê?ì\5šŽ¯?±§gâû'ø?0æ~‡[?Uàí4†"?½
m!§«¼?±¢
èw‰`AGN4FGL J0958.0+3222?ëyYnl€@J!æî·`À:oÎ=UÀ<A©î{s@{k™¬@Ý«ýIl[?¼u_þmXÉ?°ç1ýÔÉ?ðmjœV|@"ëa¸W?í™j4Q@d¿ç@6¡|¼ê¿çE\á,€<¿æLs@i|›¿ë—¬ÂkJ¿ïõ´¢‰'JAGNfsrq3C 232?ï¹VÕ=£h?r=í£Àd¹?h(£;q®¹?Z<r?Ä+`?w@CË´"d?m´Êž³'¤?ÁßU]?…4½Â…Û~?j–qݚ$Ü?rMí°/zÇ?†³sºý~?}á/BSZÈ?ï/P¥‰çË?ˆVnœvàà?xC¶Nã=T?wÿXòÿI?"ýÀµ'I?"m‰ÛŠz?ï\ÁiIù?qESþÑ?Š¶àÄ~ß)?mÏã›òð?|Q]© =?Z*™¤ˆã?ï8¶\j[‹? ª'·¾x?€Óƒ³ÈÖ³?u­yVÅ?r'HáS?Œ@Ø/l"?î‰Nó$œº?¦B8û¸?'nÍöh´?Špr/§ ^?¢Ï]Q¾s?£J¹šg‹/?îoÿ(¶úË?•®NZ̗?……ç)'=G?ƒCëBŒ?£ž"«"jÿ?'—˜¬lŸ?î35u?'¹_òç?¤°_<¼?]ïy"ø?"øÚE&ò?wJ·´ŽÉÑAGN4FGL J0958.1-6753?ЅîvÀ¦¤À$™ë…¸RÀ:ö•mºîÀ<C¾˜V£{@始ʣþ@ùPá™ãk?¿Yô›¿´B¾$=w?÷­N·ó÷´@Y±rµÕ?Ԓ{'­Cð¿ä¿ð{'¾‹¿èH4rß¿áŸÿ¿"SY¿å´ÊAؤ?œñ(™À'AGNbcu3FGL J0958.4-67521RXS J095812.8-675241?ïc¿z ?'[ª"¡^Ë?Y1èʺã?Jé¹v+e?š i0ûS?ö®d?ꙠQ¼Æ?¼´¥‹Ã?v_â<Œ?ÙÎ4ÐE?Ä思IQƒ?»¶âjBéà?î½ÉÀ
?'CĬÁ	b?g"Ãývö?TóÇãYL?¢ª'¹àêo?ô«
ý?îÓ	ȉNÑ?€PŠÚ?dØI\/JÚ?K¡¬1‰?¡Þàø2>?à»é'æ?îFù_q?¥;èÃ,Î?jټ܁+'?bD¬»^A?¬ôŸ´Ç?¤Føž?åxj—E?Ç%—´s?x€ä	t?…×'íÐk?ԛÛ~Ò%?Ç¿ ÇéÂ?ìÂ4Q…¤?¢hY¢âb?y_—ª(•?m)™ŸUr²?¸Xcù›i?¡Þ»ž½u
?ëš8È?ì¡?¡Y˜'Ðý?ƒFðÓ/ô?s¶)
()?Àf¨od*¼?¡FñÙ`AGN4FGL J0958.3-2656¿à˜›± @5Éó×ӑÀ;EeÄ÷1À<ª%s@-ÑRB˜?ÿùI²Ñy?Óû¥ˆ€?ÎrW`dÙ?üX(&·@õ^'?¦ÏF_ñéM¿Æƒ¨9¶°¿ÑߥA˜{·¿ßƒÄKžå¿æ8ßå®E"¿ïý²èõø?AGNrdgNGC 3078?ïµ÷¸U>?qÝ4êœf?cZEùåÑ?XV&—·HÙ?{Ïa?˝ÿ?l©ûÄ'u?ïCQÍÁÙ?ŒäYq»x?w'TüÚ"J?x}+p7rÍ?'µ1†r{?…Ç^Äsœa?ïMú¼@¯ë?‡ã%40?tKCiD
â?s¶÷/®L?'-ןPÍ)?zЮÀ‡™?î†_øZ'?}(ÃâÓ'e?‡r~«4T?cX‰¹'®?¨fý]_íÖ?z]4Aç³?ïb«DM%?á:G—¹?sÃ¥…0C?j<¶žôw?s\R˜&ž?|¡qk"q?îGvá?¥èDswq?_k³Gä?'}nK F?¨ƒ­¯\@Ì?¡§n¶šp?îÃâë?Ž×c"β?'2ºi>ß?€ µÖãÕ?ž"†esòø?‡v#–¿ü?ë.D¹÷6?•^¤"ä?"'#p͑|?~šÐMMLL?À¬)œº?•7)·æ4AGN4FGL J0958.4+5042¿Ë_ËñÊL@HâãK"SÀ:bŸ1‰À<²Š¬–Ì`@iÂp}k'@ûµ¤at?¾ª ¹.Æ?­s\f³=?ê×'[å@
ڧ옚?â<x¡|g¿äÿïÕ¿ço˜p"¿èàíìEz¿ëèߥ¥¿ðAGNfsrq7C 0955+5054?ïõT†•?JWA!M;??÷âLîY?8	‡/å	?L*D\Ô?AçÊxXª?ïÒ3¡m"˜?tÒªYŸÌk?K8
Ï%€Õ?U–·²âÂ?s-ÝàÒ²?pÜÇ
Ôæë?﹉-æ˜%?uóç¾Ñ?`>Éƈg$?j
àòR?{+}î?ok<Š…?ïØ\Ê7B?Qî^–N?dÈÍîÕr?HuՈ|ªl?bÛ4Î!¹I?DÙ`ðX)ô?ïè¸íiG?]aA˓È
?Nì±''‹m?BrºÎ7:?`8×Ô^-?Wìć{V?ïmuR¬9?ŽF¼n"?`,òvßkD?gyI;Œê?K·\¤Ðí?Œqý¶^'Q?ï'ê5"?‡¾&¡i?c_ÑÚzJÏ?eZ¬
LŠ?Šm†ƒKÖA?|yø<-×û?h¶·?s\¥ð,‰ß?€ ™Öêز?i«¾cJ¤?|rÚõ'?e÷sã~IoAGN4FGL J0958.4-2441¿êè
yfÚf@7|#̍ãÀ:rçy }NÀ<WË/=Û-@º+Kˆ?@	`Z³«?Áw÷ˆàd?É øžï"@È9À.e@)Ï/þuf?ÓÏ6JÀ¿ÛQc'A¸¿ÞÓA:ÝÌy¿âQ(Fp&Ú¿çñðÃL¿ðAGNbcu3FGL J0958.6-2447TXS 0956-244?î²é©c?¾wjÛ9ù?¾dn€Ó?£³	æµ`‡?™ú1Lå?µr'F±?ïS*ÚVð?Á*‰U»?x´ø0ß?~yjCÒ}?ŽÛ{Ir?"ý}pxuù?î쯁@?'PCÚãJo?F¥jƒ­?‹#{ÕðT??"ƽ•,Ç?ƒý*ô?î¨3mô-?z¶/°Q€ù?‹­jCÜ÷?cõî¨ðq¾?§º"8)¶4?v´ýa5î-?í5eøka?¼šµV?»?£ ]$•­ô?ªGu{ÖZØ?©‰QéOæý?±xVÕç?î[H·:%?¯¥ïó€[S?"¦Ë}-?žúÙâ®?¦Ïøs–;?£ŠóBë'¥?íBß"ºÀ?£‹ü<†_?¥K,ˆ¦?b–ʊ?¦4«:õ­?'éfž` ÿ?ë21Vëˆ?•osƒÄëä?žxÓrФ?9ûZÉ	'?¾Î—kï›?"'o‡6"AGN4FGL J0958.7+6534?ÕAlÓ#9Q@EYtæ[êÀ8rÐ4³À;´~d‰íT@êƒ-±@Kv Í|?"åL"C>?¢ÿPËN@BåۑŒ@¦±['1É¿·(ÃÂ>~¿àåÜhKBô¿ãƒÿiKZ¿âýò^¬³¨¿æz¿^z3οᘼúDZÛAGNBLL3FGL J0958.6+6534S4 0954+65?ïòÍ5#?I\Çq
G]?)÷͸š‡ï?Km¦)?W&œ-@?G²†)Ä,g?ï×Ú0|cm?q¬ <f?EþÄ·ñœ?S2•ìþ¦?qr‡ñÎQn?näU
²?ï¯é"¾k5?|S°²>?]l=áÒq?dð:`>×?€X#¡/'?y¦w
"ü?ïþåòdI?
'$Æý+è>óUHÇí•>âä6¿Hœa?lRtöQ?4~ßÃ"µ?ïãÅ̟ͳ?bdÆ©Ì/'?._@Ãäµ?$ew‹¬?jTB¸|Š?bL"¬I?ï–㵂¿t?Ž‡æð¼Ú?Q£E^=A?`×Z³†&?ˆ©ìF;ƒ? ˆÝx…?ïpxé««?ˆªL²D½?dOûï8ØE?g+‰]Ë?ŽÍûîI8?‡s_zV?ïýÁ£Ç?%ñ"¥#K'?*¹ù¨ƒ7>üˆÍïm?/$æ1Bˤ?$0+}oŠAGN4FGL J0958.8+7039¿×ÄC¹	ÃÆ@D$ p¹À;Çp‹ÔÀ=%Æc&@@!í³/³ø?øÿ&¡Txþ?×ÚQðœ5?Ñ${tëdh?÷ ªêúµ=@ߘ¬^ÿѪN½Ó4Æ?Ö{4©«?áÝhã³?³àΌj‡¿çP䉁ôa¿Ì.îúâ	AGNbcuGB6 J0958+7039?ïÜ:m‰?cùIؾ)?Hæ"&ƛä?B§6›õ/y?mŒR|Û8?`ˆÆQwZÄ?ïÀè3kÎk?xŸ÷+Æ'?Rðn³4?ZqJÙ4¿›?zÏʞ˜]º?t2jÏÄ[_?ï Ëà?‹*»v€hZ?lªFì?p<ÐøÎÛâ?˜cèÚ4ïj?‰	ºMu'?ï.³a¾?vÊé¬,Gt?qŸ6c)Ë?Y¡$'ԑ±?•Ö¼
,¦a?t˜²¥i?ï¶L3ùñ?u=Ëì=݇?Xµç4¯m—?LÊ4¨'v»?~Ïà)UKÒ?s+ÓOî3á?ï8Åü—?"pÌÇ×?h¹»²Ò"?s²E?•Ð$"¿xï?'¡ÀÎx?îw}Fôþg?•æRv?r¡œÉä`?qTh»Áê?¦4	ü:ö?"Ò,†fy?íÿzÚØ?'ñ߶uö?z·¦/?r(ۘxü{?¬±`JB™X?'±ÑgÉåRAGN4FGL J0959.4+2120¿Ô`¶ y¯@IH8Ÿƒ¾fÀ:§]u&ÊÀ<…='[·@€Ù% £y@"NCYñä?Àªa½à濋—/Üçw?Éü»§áZù@gNåúÆ¿ˆ@ïÎs¿ßpš1o
Õ¿áéžÊ[…¿ãgS–€	¦¿ß†3‹GÇ?¿á¹ASAGNbll3FGL J0959.7+2124RX J0959.4+2123?ïÈËBU‡h?qA½M?VÉÚìU—L?jNÉÍx:?uçè+Tñå?eŠ=ÍHþ?ïÔYwÚEö?q?æwÌ?C<ˆAžÔ?M€bÖ"%?sk²ý­
>?mä'Í
÷ã?ï†n‡OȞ?wÒ\Æ	þ?aMR=º?\à{ê:þ?ŠH`"?váÒ3d??ï®Ù÷X?]Ú"­?ZN"Í&ñ?:íXÀít_?<Ñu0·6?]¨ØúxR?Rånô?{Ö}1W?c¸gÇKs?T¾Óh–n?ˆ1Ñ}Ct4?x™'·ž—?ïl¼•¶ÏÏ?'G›Y?Sòìw>ä?]˶-ÃA'?')>†±1&?ØçÌÓ8ê?ï3 ýwK?†¼¼ÍË?p_ïê·+?lez±ã™˜?šéjÝÜ?"£¯x4?ï;àŖç?{`',ãò?r+YXäƒ/?ZÅD.	~?›
­09M?zؾ(p¹AGN4FGL J0959.6+4606¿æ­VBŠr@I¤¹#¢œxÀ:¾=¢ø½ìÀ<u¾{Ñ1¶@$›7(‹:@Róš–ï›?Â×ø…bU¿¤E_@éep?ÚµgÀÙyƒ@=Ò™™?Ú/é(M&¿á­ïýS}V¿ê^ç$.³¿èP"Xð\¿ïÿòÿf}
?ïr·bWcAGNbcu2MASX J09591976+4603515?ïâwL£ØÉ?d¬Ú3°Ž?_ºíÿ-ç?YÜÜ´&ZÙ?[þ«ÒŽP8?YêKƒÑ!?ïtÉøÔ_?›è­Ò+s†?|ur#%ü?€ü'.²\Á?"ô#)°˜?˜O·3™›®?ïV¼¾ün?‰ØèKôÄ9?€¿_obu?€	»<ñëÈ?–5`2ep?ƒ_~"Jti?ïˆbö"P?nËñŒË'?yÄÖ_Mès?bïRæ†L*?×MTש?cùü`±A;?ïÄVK'"þ?v8ۋzö­?s¿ûI·*?rŒ@ÏUΡ?d)½ñl.F?a²ðgç‡?íb¸~X—é?·|²è
Ÿ?Ò 
‹‹?˜ –ïn»?±a¹9F?µ >‹ÚRí?î_ÇØÇ,?'¨+^6v?ˆõhÕßùƒ?'Ë*÷גÑ?£ÑyOCÜ?ŒÏ¿Îõ?íý—ãa
â?–Žßɂ)5?œØ3''ƒ?z'Jª³?¡å•±À?Œ@ÈXZdAGN4FGL J1001.1+2911?›ËjՔz)@JOKrÅzÀ9z¿ª¥Z˜À<^×,¢z@wÐ1[AÅ@ä#¾K)Ê?«ÉªƒvÂ?®éO[Õ5I?þ¬5}N—@kd°-Û?ÁZê‡GÝd¿áÜ,¼ ­¿ä¾ýÝ;¿äÍi_•ô¿ã˜†t"è¿ß¹ö{œÙjAGNbll3FGL J1001.0+2913GB6 J1001+2911?ïíЖÂ
?{Ó£N'?-±
9vú
?5
™ˆyš?`TXbeÒw?{\Ha_ï¾?ïáDÛs¦?i™¬DZ7°?;Ác½Ñ?Dt¦5Um?kBøIfŸ?f`,>#V?ï·!«æ0?wój*¡*?S'ë'ú?>úï*v÷?ª   L?v¨=h™±?ïúØÞÓàg?&Åԁ3€à?$d^´‡íj?	~®¦«ö??Û\«†?#ãÏÐ\ü_?ïÜÏDZŠ?rÑ끃!?9¿Û"eZ?7b×
÷T?oøWf¯'?pþ r'n?íI!»?‡ä±27?P"€Rš?Z
'mŽÃ?†ÖÂX¥i¤?†Á^"š®í?ïgrwì ¨?ˆ	D®M?`¢ñ£Ý?\ï· "DX?ýRßG?‡KßkNÇR?ïñí…K{K?Hã~ hq^?;¤¾Zû8½?)3‹—x_?U;Æï`Y?EhP ¹Õ}AGN4FGL J1002.5+2215¿ïwð7¸ö@IÂ/¾3¬ÖÀ:Œ¬nˆs×À<wXï…^y@ žv{‡_Û?ýä(3$ðz?Å‹ypYY?›˜+§Åù–?،üÓ$Õ¢?ðÆ+«T'
¿Úם‡ý¿è
ÀGƒLP¿ä.]
¿Ô"ãQs¿áƒ÷ÜEÕ¿ÕÝÖÿžAGNbll3FGL J1002.3+22201RXS J100235.8+221609?ïŠ:X7ñÖ?™ÅNôÇÍ?O òrÍè?CXÛuF}?‹ZÎäœP?™·ïã*ÆÎ?îì,ÿÅü?œ9x"'˜Æ?¶À%€r?ˆÛ%–l²i?™žÿëû>º?"såHß?ï-îG=N?Ž8Þë=?rS»ÚD?uN%ᓾÆ?˜e~4
x¹?Š^sû¼?ì?g 'õ$?":Ûäåu?˜ºuˆøu?~F³Xµ‹V?·ÿT\Ä>B?'¡Ø£Žž?ï(ÆÍ{À¸?"¤È²?\ÚqíÚkÍ?S-ª¸Cá~?™2.3A?"mfÔYK?ìù»Ø*Ep?±_Í&™.Ö?"T·Ðâ?šQvyµÌÌ?³Ì8mÓÅ?¬1ž—1Ü?îL̓ZÔý?––:×{Ù>?£Û"#$m?FP
ÿ?§>»VÌ£.?"Å;µ˜Ç?æ2ù[9ü??­=AŸŸ§'?ªƒ''VÇg?•MÔÒì?ÐI›%FÔ?­$Ÿ¦áÇ)AGN4FGL J1002.8+2140¿Ûï›¥Ã@I³ÌcñA À;c$W@YÀ<ÂWþė@ÖZÖæ+C@˜ûyˆ'?ÊôµÉû⿦³vºq€v?Ùy3]$žE@‹ž†é=ǿ什ÿT‰o?îE¶Ãvö¿é=1ïfTÉ¿ÒUUM9¿ïªøÎÞ?åo‡wX&2AGNbcuNVSS J100250+214225?îãäÎÌ+g?¤5üoìÔ?qºò3«}?"Çw,Å ?Ÿ©›Ÿw7?¡Bg+"ç?ïÑÊô
6'?r㫒Í{?Fæÿ7ŠD?NžªMÎÈ?t=¦#˜?pƒ•°ZÃ?îjŠð´]•?™K8Ô"?y²©Oåœ?|%_¢Z©?¦ ûÈﺼ?˜˜Á ~ø?ï¯ÚƊ"l?d=ùïÊo§?^ßJ°¬Ë?FEµ<Êx?€GuñO?bU}ÐXO?îlÀ"ýu?§ œ4üj?x¨¤=¨RR?zÜôÒ@O_?«"qÐËâ?¦¤o'][?ïk³'ß³Q?
 MHc?Y2'yÆß³?c7óMËS?öd³¤Uâ?§sRÜ;˜?íLïNyW&?¡£ÆÞ8?€Üˆêe])?°@m
ñ?³|ôoĂ'? ýeŒoç#?îûy"€³o?‡
iŽ¯Ì?v$o<K$?i¿Ð ÐõB?›	ґ²Åe?"ôsS
žQAGN4FGL J1003.4+0205?Õâhm°:N@ESøüÖÔÀ;9|"NÀ<¬#þ	ù@Óy³J?ÿpŽ•·?È´ E°8m?°Ü_çÇ$?å•ò`L–?ÿµ³–??ïî"%âؿꐀýÁ?³$œ—zÛh¿è¢JBCqo¿Ú¹#ã	$A¿‡.tɉ)AGNbcuSDSS J100326.63+020455.6?ï•nёO?€€ñÕ4mM?Lovà{3?@Šv¼'`ç?ˆÝT,È£?€Þ»|X?ïw¦äZÞ?‹qÒ«3?inêƒÀä?kÅïÿ?‹ôz¿ÖD?‡«Ù¶_æ?ï95'\ªë?"‰ˆ™0?d8GDç(?TX0IE,©?–RFÒTÿ"?ƒé_a²Ë
?ï©ñ«~s?u$B`ìä£?iã'Ç5.n?TeåKeò?˜î\Í2
É?súgßÁ#?ï
{'ƒ·?'ý˸'¾?Wú"0N&?KÄc÷œô?œÝHñ¾?'–bvz'>?نˆ_?£ùØ4C?tËîZâ?~Àf/‡?£=ÏãÙ<?¡Vù*ᛊ?îwzÉ°ô»?"çS—8?n}\.L—$?f&èÿŠÈœ?¦ }£ÌÙ?"M+"ü=?íYáÔoÈ?"'»Öd¹?{¹;Vât³?p,Q'"é?³u`<FPs?"¤ÁT™kAGN4FGL J1003.6-2137?Ð-4‡Ï @:ÐEþÀ;ŒŽ·¾HÀ<À
(ÝnÛ@"ÿ2ûé?ùú5 Ë½?Õ¦_»&‡(?ÀJ
MzÝ?ëbC¡ÀY¢@#fón¢¿éaßî聿é/"þ)f+?ï:Î2'šy¿Ø7±G5H·¿Ø5H Öj¿×A¼ã˖íAGNbcu1RXS J100342.0-213752?ïЛÕDPÎ?i´°ØAÎk?7»|'n?(P_U[j?v6cJohW?hís©?ïÂXî6\'?TbÞì'é?NX³¨q×?Z]­)ðE?{r|ã˜#?züI£øA??ïN^ë0v?ƒ"|>÷Û?Uf¼ëŽ?BObÑ~½ž?"ä'€yAr?ƒöµ'œ?ïbøÃÔ3Q?p¨y£0yv?=÷*|J2‡?.*_*]?")
Õ	öé?p˜—
¨
…?ï|'Îb4d?"'™²þvf?J …℃??1^Gå"?>j[Ùé˜?"	E±cÍ?ïTÎLg?–ΈŒ÷ŒÎ?_ùªG‹‹?qzîÝꓟ?"f«ŽATg?"oÆ!N?î¨ÃGß=?'³ì×\?[Æ.°g|?Yaíô a?¤•šŽ[Y?'ƒ§ô_?îNÌÃVp>?'BçáD5á?F/—g<¡ù?D
ꁪ͙?ªºulŸ­³?'/ˆûŠÏAGN4FGL J1003.6+2605¿ìMdø'C'@JTX`fÀ:›k¯{ƒ.À<wú ø@
?h ¨W@"¿'a?Äð!e«U"?Â3£Æn8î?÷O­¢e6?þš<â(¿ë{L§xn¿Ù2ñ#Ä*g¿ãrZ?çvœ¿ç[§J¿àÑ۔æ¬r¿ïüfM;òõAGNbll3FGL J1003.6+2608PKS 1000+26?ïaîuF±ž?¡¯¦èŠä?jÙZõ#?oLûƉa?gõAÈé?›+m§˜ù?ïR5¸&U2?Žü—
úÉÈ?rÉÆ#
ª?qùI!C?'4ւui"?‰bïq9¢?ïD6‹Wa'?€Ò
ªÐÈ?s/Ú\±Ÿ?oՌl;?'­8'á¸?|Lm¾ÛÁ?ÅsMf?€òž&÷›?kÎaË:?q0ËÜÛ5b?ŸÕà–ѯ?{*Ք80?î'Áã(?šæ†®Æ¬–?€6€F¼?{ÙWdL?¢ÖA¾Üâ(?˜§»´X?íËÄPɾr?©Ç›–')ó?Š´@e«?"§*îïv?¬¾MânÇ?¥óÀû³??îšpB?ŽqQíV±È?~–»È2?vI«©_è?¢\<¶ý?‰ƒ¬BŽ?ëãÀ8"Ç?MWWî?¢£³xã?uðÙ,½´?·•ð@&É?š"άàn AGN4FGL J1006.5+6440¿¨Á°õ6ë}@F&¯%;À;*.XØß*À<ç3cښì@ ÷êÃز^@©}'Ô?ºrzù*¤¿¿Õ€r'?òXåªda?ÿã­¹â}¿íÐQò;_¿á½c£=‡¿â\ᢜ́¿ÖGKCdt¿ä	Úÿë]1¿²zs8±ÍBAGNbllRX J1006.1+6440?ïu2T"?«§qm?Nü‹l€!?B£ñ&z?aÑ$w
?«$q !¿?ï'ïÅ[z‹?‹IÄé*?`ñ$®?hží<Ã"ª?‡Gʱùé?‡³;C\}?ï6Et±áB?‹¶³.5à?_!"hÇ?GŽ÷Ymâ?—E9+VN?‹&‹Ð›Gö?ïSƒñDXþ?}Käw"Ö?vo8W??^˦çGèÆ?	»s;¿|?}­þj#–O?ï¥!ë•Ã?"Ÿ¯›)4Ù?bÙÖ\ ?Zó2©€Ûr?‹`oˆL_í?"dŒôá?îÖ©'M3©? d§Æï?q;G³®§Î?vsýýßN? mýñsOw?RÜ°jwŠ?ݙ›?'Aã°Ø¿?i¼¹ûØË?g¬µ°DŽ¢?¢øƋ LT?'ؽ÷f??íf~‰%Œ?›¢Š{eôH?"^Vq¬?…0V''p3?¯fýìŸA?œ­óBØAËAGN4FGL J1006.7-2159¿â›6®¬•@:Æm½r¼¶À8aKŸŠÀ;ÊÊ·H×	@ê'1È$@ZaÎQ1?±!ð@+?§Œ%'¶¦p@хÞz@¿´Û>˜¿ÂŠºX«è§¿â}Wyc™-¿æ8"œ×%¿äÙ>ö
¿äìÉA|÷ø¿èw]š
_AGNfsrq3FGL J1006.7-2159PKS 1004-217?ïó§&ŽÏ?ešÉiEŠ?(Œ®>?#¡HÞQ|U?VáÆ>F?d«ùj?ïçM±ä"?h©¯ùƪ?8lÇaa),?D·Å\}z£?e¤´üˆ¾‹?fµ»õúB?ï+w°™C?†ÂÔIšˆ?]³1+?j;Þâ%ßñ?ˆþ»Þó'ñ?…MNzQùÊ?ïþ½ýžs@?U.'k>ï÷Uw/fc>ÞZ•¸ÐïK?" ³WyL?úæås÷?ïË7F›Î?…Çï ?7}?eš?:Ø\dÎÖ?xúy'A¦?…LF¬A#ý?ﵪeˆ‰Á?…@Ù¢˜þ?P‰èÐO?"?bÏ¡uÖzÜ?€")"Û‰æ?ƒÝºÐ´Ú†?îú'6X_E?˜!m©tÚ¨?bM"ùLX-?aì¤ã_št?žqtÝ-µH?—¯+ïJÁ?ïýR,·\è?*ÿ¨ÿ‰['?ÏäÓ
µ>þçÃlP?3ºð&ÿ(?)C(hwqèAGN4FGL J1007.0+3455?£Ïò;Q½@Kà?pÀ:š¯_Ô{îÀ<Š®¬Ÿ0@ oè;=B×?úùcc|§?Ã#öiÔ/?Á*¢jùs@Òz{Ç!@g&q÷?ïÕřҤ}¿â†ôæÇIÖ¿ËåÛf˜Z¿Ôñ§ãxu¿à ÇuË¿ÞE`Ý:ƒAGNbll3FGL J1006.7+3453EXO 1004.0+3509?ïÅ^@Óó?kwg}+<?M>^j—&?=¿«·?y®×â‰0n?i¶P÷ÐÄÇ?ï™Iø?Î'Ôþõ?`½oJZS?_ÙéÏì®Á?…¨'°šˆ?{0àû´h?ïuz­'—>?xi
?`Ã0yîü?L¶´®%k?Žpˆ‹ü¹T?wX1elÝ?îtÜ;]VÑ?x4ý&ø~?ƒÐO-¥­·?aâ!ä|yø?£¾(€bø?uï'f]?ïi´…'?~úØZ•éß?bâ6´¦Ÿ?W€Ž¸Aˆâ?‡mNäãœ?|Iycø±°?îâ²hXÀ?™‹‡}ÐIá?sùÖY4B?z5‰¿7??ž«=YG‡
?•_¶"&B?îø»`œU"?‰\ w«Éw?j_SB·PŠ?^¬6‡¥?œ©¦ån?ˆÿ¢¤¢?ëõ‡Çg»¯?"üèéûì&?•d?îΈ?|7=DQÂ?ºú±È ©j?'r¼=¼ÕAGN4FGL J1007.6-3332¿å
"4Ïã@1õßeUÅÀ92 
¼À;ûN']Šö@¶‹¤ô@<ï>çœ\?­ý"ÀÁќ?Éü§ZøI'@ÿõbLM@÷Æ0{s?Юý®ìè¿ÞÁ {öpŠ¿ær¡Þ¹¿èkˆVÚØ¿éÄP'èË0¿ïÿÀtϵµAGNfsrq3FGL J1007.4-3334PKS 1005-333?ïoWs&?¡(úþ–üå?—ˬ1
ùo? Sgîí,@?z͗•çN?t‰·½Ë£?ïÈú‹)œå?|-ö7u©?W,êph?gó&N°~™?u·ÆÒ<n?sµBéEë¨?íºiŸù&"?¡¶ñƻ?£óýósE@?šÇ»`ü? eh
Ö8y?˜)€
Î1?ïУPI?YL¢¬{G?[aÖ	è†D?EXÞs\ä?pÕâtz¸o?R":LA$?íãº"
¹?¥€øËç±?©¸	xþJ?£àT¬B6?ªš¨^?†+pœZä?ïgńŒŸ¿?šemXÈ?köê>5'?zÊú@ð?äZ±G"?˜ŽÔ>')?ì̱ýŒ?§zÊ¥Ääæ?¦ž]
LCÐ?žI
~ìÁ ?¬ —âÊj?¡Éå>m)ø?ïw>¥¤{?veÌ#ƍ?s?¬>Å?`ë­|iL?ˆ£»Vc×?rdè¯mAGN4FGL J1008.0+0620?ß,˜ú¸B|@G×süÀ9*¼ª?ÚÀ<¼ bv@Ù'ÌLÊ3@B+{®Í?«0ªþ×ó?¨)Ûúë?ü´d¬R@ºË…$?ïþ[à¦sr¿ÎBßN"¿ãíÔï°ýc¿ãˆ¿V"¿àºÇ犾5¿èZ€êv+AGNbll3FGL J1007.9+0621MG1 J100800+0621?ïëtöªŸY?q4Јmo?*{¾W!"? LTœ`7q?bãM'1+ù?q#ƒöÌ÷?ïÛy¯³%K?n1™þ2é>?@"	ŒØ:?IÊ{8qÛ?p0¦ÛˆfÀ?j3ÀmŒ)?æíW?|ÒجÙ?\³/
8Kú?`X+'.‹6?…yà˜eúÌ?}õ]ª'?ïÞÓ;+Ä?L¢0›¼¤?T8äƾ=Ü?6s…üãNÇ?gRoxݱ?G{dïZ€†?ïß´Þ¹?g÷"±c?5( ÖeÊr?+ýOÞ¸ŒÔ?nD6ò¢¢Á?g2‡]9¼?ïŠþø)X$?†Ú	¢öL"?V¤l°?aÄ´?Šk±ÈÈ,ë?"ÑUhTa³?ïm&Çȉ¥?"Lji8Ôa?c<üàèÄï?dàÅPwSÙ?çØ»'?'µb³—‡?ףּz¸X?išµþ8?iÿBáÚ?U
'ú?|>¸Z£‡S?dLvõ+šöAGN4FGL J1008.0+0028?¹L	Cbº¼@EO'j@À:O{ûùáÀ<n,·/¢@1¡&@&býüÁ?Ì-µÅÊ$?»¢""EA©?÷'!A™'"@Y ­ ?ïÿü¥¬¨¿à"ßq?¿â&±$ÿà4ÚÓÍ%¿êø×ý­j\¿ïÿ‰XAGNbcu3FGL J1007.8+0026PKS 1005+007?ï
UÒU³ø?'	ö‹Oq?q+ÊIÔ¤?fvÒÈó?š
S(°å?—yIf'1?ï—æé%"?'*"Ä›åt?fuÄt°ù?kâ`¢Jß?"¨O솹?y¹Öºß'?îµÄá#¤~?"0êwVæ?'bWMmÁ?'Ï
Í? CXŒK7?'=µú±ý?îµ]Àƒ?xóÒa>2?'¥=6£Gq?lÔq, C?—¯
¼hó×?q11Xñ'?íþÅP_F•?¡~­þ'#5?"4ú\Hr?{L
y9Ž?«¨ºÄ˜"?ŸãðF~³?îÛ¹¹—e?™6gÉ|†?y60åb\L?€èîÊGV?ž;<"š??"ïØ¡‰€†?ívVM`þ??žø,\½Á?qWe|0?Š&Åä»?°0÷¼â	z?šøRµÐ ?ì˅‡hêz?'CîIý­ž?¤³E
çyj?…ª"'?®"b~ùzî?‰Ä¦-ƒ"AGN4FGL J1008.1+4706?ïÁœ}¿ì@J4ÿëJwÀ<	zP(6€À=!iθ@"tRBÂó/?ÕÑȽ/v?ãj@ºˆ'?ï
{é…j@1¤Òh@|<yX¦?ît#=qÐ}¿ïÿúÁҝÇ?ïÿÒ†ëA¿Ü9™aܔ?Çaû'©¿é- qäAGNbllRX J1008.1+4705?ê p"|Ø?Ç®Rq> ?fþHHWØe?l_NdÔûK?ÇE…§#à?ǐ"t:ÜÂ?ï;Öƒó??¤ˆ¢+‡™ò?r¨û=ûÈ?€'±XÖp?"ýÕ4M°$?¡ÔÃ<\_?ê?¿Ñ€€?²"Ò}´ã?"SCMww?‰•—T»†8?ž°Ì³nÏ?²¿«šJ?R?"¼~€35?Al»ã‡î?9ð(ž9?¦Áí5Ý?"¯åÎrÏ?龨¬Çc?ÇãG,å;Y?{Ãÿ»5ò?{ûuR¤©ù?È,ÁÔ÷Ç?ÇÊyî%'?î4ªe*?´¶	pmÜ?'ªîmè›?•ÙŠ©ð2?¨
ž74é?²½6¸Àÿ¤?èRÎ. Ð?·8:2º'?"ü8öÆ?‰îï¹H?̺uA‹Ä?·H,"š.?ìùӎ"¦?«äq7³r?7ù¤¦X?Cւú…2Î?¸G}¥Ä·?«áñ|M'*AGN4FGL J1008.7-2909?Ð:3¾°@5ŽÊW§†ÂÀ:Œ½½eP½À<ZTtÌZ·@qgd"(@ic¦˜…?È
£‡"S?̦C̪ï@€†
 z@
Wr,Ã,?ïÿÄ}îB¿å«fJ¸¿æ'F–½FG¿ä‡`F'´É¿ïý.>Åè¿îŠøìæGÈAGNbcu3FGL J1008.9-2910PMN J1008-2912?ïÜEÁ*?eºþ1¦ÿ?T—\gÞÛH?M^ä8ñ?io6ÒK¨$?aVH­_‰?ï"i!4`¸?…ƒÈ		78?paiaK?ríÉk?†µàúO?~$®´Sœ?ïU¹E™?'Jë:êðK?{ɲöhÐÅ?'8HòfR-?•'ܝ®Ã??')GRù?ï	°‰[o#?r‹(€e_½?‡¿G»ñ×J?dGí‹#?'êJýxgû?l©Ëݺãó?ï«a3»](?{lqÃëÀl?g²;ÿó?`tRòvA?~Îâ*öÜg?w!n,µíò?îìDó`F?¢)j€ø?ŠÞשY1?"~Î5Y]|? 9…Ä»áa?—r´h×ù´?îk/<-®?—Ùrišr?‰?Iʁ÷o?‡à1ÁÐ?¢þڜ0\E?"i/ןi?íQµn?'X™®™.Z?¡¦ºœ!?"^6P¥Þ?¬÷t¾?Šä_šØ#'AGN4FGL J1008.8-3139¿ï"ÿ	F6@3˜>BZîcÀ:ç6žËÀ<•ohm¨@.tûª…Ð@^ܙÉjB?¹ÝâHßí¼?¦/³Ýù¬?íF¤>¹#M@Tóe轿âÖ÷ÞshX¿ä>Sü×W¿ã/c?•l8¿åú,hJl¿àlk΅3±¿êº¯"ÖáúAGNbll3FGL J1009.0-3137PKS 1006-313?ï{±ß‹–L?°ÍŽq?b˜ÀìDèb?‹8öž.ã?ŒmWÔú¯
?¬@á¯xw7?ï¶#Cž]?xûmMN%?V–ÏÖê¢i?\`ÔX=Íü?L:Tˆm?t|¸b\—?ï4½Íç.?"ˇh5?püÁ'Å6Ä?iÖG¢éh?•)ÝhϘ?'­9'ÈÊ?難°bß?t€"ÂP0À?qˆ‡ó†ÏW?RËŸ›Â?›h¨évYV?s@|N‡…ñ?ï,´z+Ñ?Ž'v8+ð"?wô"s"Ä•?k|iűõ?™ý`Ì5»?Š¥›
¥?ïjIõÂd?—x5yg(?m!qP
•–?uœ×;c¡ò?™Nˆ˜"G¿?".&'2Ô&?íþÿ4±–?–iƒ'¡KÍ?‡PDr?}ûØA?ª;û˜b?"ªwA'+?í#MãkRg?"KŒö?‰Q§ ¥h?rŸ8Ö:}¸?³»\§}?'?jžæRAGN4FGL J1010.2-3119¿ï²	Š‡@4äy'¼À9"pæòèÀÀ;úio/bÄ@!PC÷¦•+?ûã#·;k?²'rásøË?'ÒóYçl?â3òí†+@
!"}ö¥ä?ÁrI«7?²L'S$¿åŠÛá<ÆZ¿®æ¤ o¿ä¦],+6¿Àf‹û r;AGNbll3FGL J1010.2-31201RXS J101015.9-311909?ïò&žœ°?U'DÉÒ×?)"|fD?Å? ÿŸ‡?X•"ºÊ?T*ø€G¡Ÿ?ïۇ1¯qê?s2Á—¾8ç?G³Ðjy?WÈ4—ݽ?n·¡‡ó«"?o¦P»G'?ïEéÌÀk?Žñÿt/uæ?WNZ©ãI?WdâbÍ3?•Íà·ÕÉ?Ž¬ÂÙ=z]?ïl¾X&þ?o°Ïò˜L¶?_¦ý€ï&?EïT›_Òÿ?mÅ%D¥O?nGtžUË?ï­ä?Xô62íï+?21pƒ–?'—;m7?^bL—…‡²?Wú¢9³?ï¤I•—£Ã?†I÷
Ñ?T7뚓wÀ?dÿ|Ä ,?"f,óì]?ƒ·*d/¼ö?îÑîÚ¾§ñ?—''£{Þ?bV‰•e»o?eà[xhÇ?¡»©¸ñY¼?—6Ñ'™YÕ?î…± °
?‰¤4­O¼¨?v…ssG{ç?db³Pg]?¤ß|Hnç?ˆG˜RFÊAGN4FGL J1010.8-0158¿³ú'^žÙ»@DÍæÿ}úÀ:$<ù…'À<UäíU@q"–ØÊ@gÅá÷?»ÌBŽDü´?§M༠ŠÃ?è®~F¬ã@	–­…èÝ?îþê÷Z?¿æxK5ˆx	¿æ'bO*‹¿ãqYßofÀ¿ïýé:ø$¿ï4v"±ÓLAGNfsrq3FGL J1010.8-0158PKS 1008-01?ïêo ¸öñ?]Í»‡o"h?I"<@Ûï?CVïU¾?^—­¯M?WŸ%Ä
¢1?'¡/Ì2?ãx\''?]F]iâü ?oä@ٕ?zj—ýÒô?x_§3ûÐ?ï¾Fr]É?n'|ó#VO?^µÂqŒŸ?c´¡@W¸?y/V"*0-?e®~ü´ïÕ?ï™ÜAL?e¡àôM?v³/	ˆ_û?Z}¡PP/,?|¿â×ƽù?Y£'‹;´?ïÕÂiÇnê?gðB ?ZÀ¢&üv?NXŸñ"õª?lÝEwî?d‹‰Ú‹‡?ïF†q¶?™€«JÁÑ?iVú°\n?zù+[=µc?"¯Þ]  ?•Ó‹Ð$½q?ïŽàh¾ø?yô4€G[‡?dàîC€º?c
ãmÐ…?‡Â`zM«?uæNH vá?îæ¶æºg?'Ó¶˜Od?2¥E~¢8?w)tñÙ?'ö}èfšä?w=Oïg
¤AGN4FGL J1011.3-0427?âôî´©Œ@D
êÈ`V'À;R%fÁÖÀ<y_×Öì
@£òž­œ@Òÿ#a.?Õ&¯aû?ÓFÚÕùò?ü¶¡|¼ê@
™«Ã<Ö¿×w؞è
¿å9£ûkq¿æ€Éë£R¿åo쌅´à¿ïýÕ{Zi¿éÏ
í6ÐAGNfsrqPKS B1008-041?ïÛ1oõÂv?cìØÑ?Qž	u1 Û?E"ùåT¶ˆ?kÿ‹k!™Õ?`4÷W1¹?ïºwâ(˜i?çˆwï¹?Ẇ;ÍÓ^?b֎	HA?|Ðí Î€?~œ¶Ÿé6?ïGŽÇ%{?‡ðî­+Ύ?qXìêÊDÏ?kºŸ.í?'·ëßϘ`?…ø³º¿õr?ï¦øçª@'?a~Ü3+?a£åmo/?D~Wk˜Ü?ØÌþ4q?]|<?æպ?|œÜ}B˜¥?^Pb"ÉÖf?Sñx…OC5?ƒÂÑAjÊ?z9­2/¦?ï7$@Ék;?—Ï+cëhÃ?lâ ‰'€?{öR-ÿ˜?•3Ýj8_?"œ=ˆ­«M?îÍì"ÖOò?" "´
?wÓ`›y?x³k…@ª? @¼YsJ?'ÀÞ@¸bû?ï/¤!L?€.f…É?q¹Nᩙ'?_ç–_"q?šFX¼Ë?}‡•¥ä²AGN4FGL J1011.6+3600?íL*R¹á8@KŠ($xÀ;%t…
À<Ú\ђ.k@)©m¢ñ@"õÞ>Y?Ë|¢¨a­?ÍwY}ʱ@A@š$?÷KêlQ¸¿ßC\¡¹Ñ?ïȯÑêBÿ¿ßG.<ÔF¿¿ç™mYŸ®‡¿áó:u¿ïþ®üØ-SAGNbllNVSS J101147+360019?ïqßjքÿ?'÷pŽ¯B?hqÈü%?a4Wc9I?…HÌ?€þ®Taå?î¸ÒŠã¬?Ÿ2iëžL›?ÃùX_×E?' xíïc?š±îؘæ?'Ëԉ—‰m?îqm‡†¶W?•Ï»ËäN?¾âSqÂ?‹Ó8´—ðÏ? ‰¶[HŽ?3¼&(·?íB
o™?'-]عš4?«P¡õ\Í?îÝ
¤½Á? 2΅ö?€žæQ܀D?îò®`{ô?QD»Ü?zYY—†Óô?r_[ìûƒ?›݋¢}?C"lr³À?ìLHâ?·›×èWï?¦GY‡?ªp·ŸªYú?²"Ò-•j?«ML¡É?íišè?¥³ÜW:l?¢
õ¡'FA?›{«öÆú?­›p­hã¬?™öÓqÜ°'?ê{ß' ?¦9ÎTw«§?º«J–¥?¤¯á(«C0?´á»_Žœ?™}Zœú9QAGN4FGL J1012.3-1232¿ãâ¦[|†@ARÒ^Ý)À:Ž-–;@HÀ<Rv'=\'@̀½)Áš@l dŽõÒ?Àƒ­Éý9§¿¢ûä"ºü&?á Ÿiè&@˜&+ô¿"Ów¤É›¿éÓïk]F,¿çç	Ĥà¿æ¿¸èz0¿æ›}Ëú¿®04âF÷AGNbcuPKS B1009-123?ïÙÉȾþ·?jb¥¡Å¤?Ndõÿ=‰?AbŸÃ[­q?nœùŽälK?hUö	¼¬@?ï¤!…FÑ?«um'?aš€Î·S?fÎHK•ú?'¶0¼-ì?y´]lþ8?ïA),Ávz?'KàR6î?p%¥V?k'%nÞáÌ?"×ÐýW/ò?€ˆU\Ó?ï¡ü¡ü"'?b£¥&¹©å?aþOMŒ§?E™ôÜLF?ƒC¤S¼?`HÉu9õè?'än?"'è|)?bä¿S…±?]³©ô'?†\+­‹q–?'>ýTs±"?ï-½AX?˜¡Á3eÍ?p¿Æn)Ï?y°UÆLªO?›7êSП†?•rUíNJÜ?îidvæÕü?'/­$ie?€1NrÑô?wѸâê¬?¥]dòu¹?fVÙÓü?îÅ7ž–U?"©6hÉwk?±8$¬?l5â »¶?ŸlÄXÇÝÉ?®2ó'GbAGN4FGL J1012.3+0629¿ÃØT"*‹^@G~´À9v¹Ù«À;Ù;,ü¸M@ú£è'M?ÿ"~b®–?²äv6¾/?·åøÂÉé™@ëíœP-?@fŠŒ¶\H¿àÙCӔ¿ãsˆÃˆ€m¿Þæ×¥mã2¿á!‰¢«'¿áò] D-¬¿éçšät«AGNbll3FGL J1012.2+0631NRAO 350?ïæ̅T=D?Yœö<}è?B¦'œ'¾?5Æ;p ?d‰ÖYȱ%?V>Ê^g"Q?ïÆ3â@ã†?u[IWWð?S¸Ÿ™ñ?Y¨<Úç×?w÷æò	¸?pP)o,a?ï¦aã—6	?s4Uý?a™5n=t§?cðukårà?'9±"œŒ?lü:8I?î®Fñ`â?~Ùtõþ#?w™K:Böe?TáG¥%~î?¢(gŠû1"?{ý23n˜j?ïĞÈÍ?rkϜ3÷"?V>!b,å?Hã
Uš¾?x!u,'.:?pgLÿö?ïCHÄêÖ"?"€Q•+?d×õõ¡?mÛH¾"¤?"ûè£çæ?'ºö³"??ïXÈÃu,Ÿ?†…dì.`?qâž?Å°?vèy¯Ñ	å?n@Z>ª?€UXJŸ;?ìä/¢'?–Îò–àל?ŠJ~àM?pŸ4Inð	?µœ…3‰Ñ?•þ®8~äAGN4FGL J1012.7+4228?ᝒwë©@K4ohÜÀ:hÙÒnÍ=À<v½ôµ@ Žòµ¿•?ükWfï"?Àš<VÈ? A>â?á/WK@鄈»Oø?ïä]ý⎿æܬ1&é¿àö>"þ¿Ì¨µUⵗ¿áÍ)HÎ¥ë¿ØüŸxUÒAGNagn3FGL J1012.7+4229B3 1009+427?ïáˏt?]#?(=??sGÚ»÷?-k\æ§À?jF~{ÈX¸?Z»kõÕÛ?ïÚ[JuçZ?p(?7ñŽ?AoÆ[³~?J,fo['¦?p¤b»?lYYZ]ÈI?ïŸ<Ÿ~Ç?q §ÂÝ?U@#Se±v??Õ!Ni"Ž?…ˆÓªŠÎ=?pÑD‹_A?MŠ¼ ?c[ÀšZ?`󕖱.?A\3·æ1:?†˜‡DDk?aèםÊс?ïÒ#B­Ø?gfÑ.ª+?IHrp€šN?9M‰''½#?sÒà½oê?eºÂáÌñ-?ï…aê¼Ýþ?ž»éæé"?SO}¤m•?]ì''Ù?Œ=•«±Ö?ŒÛja'-?ïF_JñÉd?"lÄ0ìf?_9‰›˜
?]
Ï)Â?•@~	3‹?ƒQ·µ:î?îáʕôª?}mN k?tp»@±ï?\n'œŒËz?žª§c$Ë8?|ÃV¤AGN4FGL J1012.7+2439?í ¿jäzh@K0ñ€
|[À8¥î'):ŒÀ;ç(Ag©]@µÐÍbsé@ZA*2?¤.OÊkI?Á¼£´Ð'@æ<à[@aÓNq'?¡-àõ	¿àlh'î¿ãàoa6Ñ£¿æt -œñ=¿ì‡!œ1ú¿ïÿûÞ]BüAGNfsrq3FGL J1012.6+2439MG2 J101241+2439?ï¢óS¸þ~?u¥œø?wÍõj"?vãã'ÎÄR?v¸`®gn;?rÔ½z«!?ï­nßê??€Ïs"F(Ž?]9Bt]Ó?mo†RAyÉ?€ý3|ñ ¡?{.iŠá,š?î'D͏jl?¡åÉðdܗ? ‰0óøë?šæßI[{—?š»$¹?–îíåÊj_?ïëÐ%ÐQÅ?Jjüûw/æ?Oì5ž¼ïP?;U¼ÚQ¢?Xi™±ÍY?AH@ê•b@?ïU­\!DŽ?Eèëː?†TŸ+¹H4?†e¢{}j]?"@	Ì,Ìæ?€z8ѽØT?îD†?›eŒï®G?pùM±Ö%¸?†ËM8E?˜P×8)ŸÞ?–oªÒ°??í¹äê>¼m?¤NÁý7?¤¯>VÞÑ5?T· ïâò?Ÿdæ³õ?š;iÁu?ïÍÖdGŸž?f^áÏÎ?cClÄ'ýj?UäëX|c–?næ.¿þT§?_wü«¬«AGN4FGL J1013.3-2551?ïð¸Ú|Å@8Â÷ÓÀ:¬l){À<L-ë˕•@Œ	K¬Ò@'óUÎ?̚Ïú~¶¿?á=ö¬m²@ø"5´í³@eyœÞ?~[lƒr¿à×ϔþ)f¿èxQJuo¿î|?k¥À¿ïÿÿ" 5•?ïìÝxìzèAGNbcuPKS B1010-255?ëQÄó†í?ÀW.>p—Ü?¾ W4*3?¿˜2ѹp¥?›^j‹½w•?œOˆ‡By?ëD©­|ß?¿D·]Ä?·«CJüL?¸–Ãð«m?¬^ޕs°?¦ñ§Ö%ð?åÿĦ¯?²úH÷ÑÄj?ÅxùÝ˜n?®+Ǥ±à?‡õéaê?©Þvøú‰?ìUk
XòÏ?œ"Y[#?­¾ÀF`õT?'•žY¿0y?¬êŽá|(½?Žn3t
d?éj¹`£¿?Ėˆ,´¾ä?ÃênAë̆?±ýdU{C?©ª°îúèø?ªäUÆÚ:6?â¶/¡z°î?ÍN…ÌU?҇æ˝ð
?Ë¢+IÀúm?ÀsâÙ\0?³=m"p}?à̆•[?¶LÐFI¨z?ϗÏ#-"?´:vçpš¥?Í7à'¸?°yÒ[Bv?ägEv¬¯¡?³31åé?ƺo>ɋÇ?¯‰µ_ìÑ?Ǩz惵µ?§XGҘAGN4FGL J1013.4-4006¿í¦,µÊ<@*ÆÜ~ñw§À:z6ó²äÀ<VL¹6£@]U¼ú@â@ÐO8?Õ7¹«?Á§ßÐ?ýxZŸˆÆã@Aï"¿ïðõkQ‡²?ïmÅÖ8†Y¿å[¿¤Q¿Ûìü=3g¿ä\°ºv¿ïÿø¨ó©°AGNbll3FGL J1013.4-4008NVSS J101319-400549?FÄpÄ?}Ÿh3oÁø?cY‹jäpÊ?[ùù-Že¬?ŠC‹gt$â?z³r7–Û?ïepóI?Š=öpÎä?a—FR©«ð?i‰I‡ãÛ?"@Ò%ü¼È?†I˜ªzJF?ïU¹¸ühú?€«BÞÖË?h0Ž(N?c(°'á?'B°"V§?}iqX;ç?î͂žo0(?w¥ÖÍÔ?"–* ý?bùŠÇÅÞ?œŸžºõ?sÆÛ,ƒ)?îßJ'ý†?"°ÿp@¸?zgO¢*£?x˜•'ܐ?…'Ó‡æ?'
Ç^lÖ?îÕµÑބ…?¢+
À+v?u<›ÉÂÿ¶?'h/¯¿"?Ÿúזd? SAÏ
ó,?îdõÂ(Gâ?•ÈkVI¿?yš<N‰S½?pͨìà^?¦}\V€ì?"Ù˜|ͬ?í1/ç"?'RÂ5Ÿ=?˜?—¦—‡Z?v1a´?±–¯'&?Œ‡0¯wÙAGN4FGL J1013.7+3444¿Ì-oD0††@KÉë têŽÀ:2Ÿ|àÀ<o©æ÷n@,­c%`@!þÍ?¹?½CW¾ä?ÀoU®2X@YO?Ù@R5£zîß¿Ó3ўm¾Ê¿æwÏz&6Ë¿åÙ¾bPØ
¿êÀÄyA4¿ï÷?œÎ€?Âø<èÎdAGNfsrq3FGL J1013.5+3440OL 318?ïð²õá3?S9åJWÈ??™É¶Ø?8ðAKšÍ<?V³¢En?ND
PËQY?ï¹^e»ñˆ?}3ëö î¹?Z^="B?c"ëA|?|¹=º$ób?u¢Äa€é?ﺆЭñ¯?p"Ð@–r?[¾OüÒ?\ù¥Mü?{Í'$á$?m¤ùrô?ïÊnˆ@MD?X!cwՖÎ?gáýýñ"?Kò^™?n•ñÏQÁ?P×HÃ<§
?ïÓvxh'²?€J&BHŸ¸?Ye=E—?bE]AK'6?pªŠÛ£C?x­±˜W¾ó?ï9´XÍ?–ùüß#?jhÚ¨ç+?v'è™±=?•|Rã‡h?"?{5ÃjÕ?ïq#óiš?Mg'ߐõ?gFEÝ Q?eÓr'?­?åq¡gu-?}Ã38—L?ïJ oäû?~í&|ht?"š*'5¶?q¯Xª…ª?‰;`u­ùo?sß¼ Ö±÷AGN4FGL J1014.3+4112¿ïÕ¼Ì	êv@K{š¿4À:'7褙¨À<"þ)f+@{"Œ¿k@	ÒaaCè?¸ºt_Mm¿²æ I»O?ön"¸‰Hé@$Ž³°F¿æZùý‡€¿ãŒ¢~š¿æÈZý|˜¿á7ÏÆl`¿ä"'É›À¿ïú®‡ggîAGNbcu3FGL J1014.2+4115GB6 J1014+4112?ïòAtz·g?PÌ犢_®?<ü»ò_Hø?1Cs3émH?T=èzF§ã?L'SUŽ¼?ïØ1œ|šR?p½#ÔöÝÝ?E'ÍnÉ9'?MçÀŸ*‹1?qB8&¿‰Ò?l	Á#½?ï´BÊ!n1?q;Âb‹q€?SK¼Ï?>ÕH)Â×j?€…Ïué"-?pÈ-ÿ‹F¶?ïÙ|¸Yő?QԏgPA?X°—ƒ2?@Izя´?jso Ž5Ñ?Mã×±?ïæp彬?a÷-…­?JCÞ£"£¾?=Qlüx_?cm—RÚ|ë?^åå(ä}?ïzÎdm?ˆýr‡?Y­ûØ~]à?`³]»¼?Ž§t>9x?†Í7Ù?ïqævl?}4ï®H²1?aØ"ò'-?a}¹Æ;'?D=±6Oe?zçË`#Ý?ïz[Ó\Ö<?u‡8Ý°ä~?vw¦oâÜD?eSL"Á`8?†-7îRÖ?p¨»Áž¸AGN4FGL J1014.7+3210?ïñd³Ö(8@Kâ­>'À;[HŽå
±À<ÓESÇ'q@ x|l75Ì?ö»Ò©…Ÿè?ÙV»"«P¦?ØmAKúªV@cS;ç6Û@¤tz{FG¿è…¶Æ'¿éÛÐ`U*T¿Ü€("X"¿¿¯'ÿ'¿âVbýüÁ¿ç½®(`qAGNbcuNVSS J101445+320725?ïâÐé"T$?acà"ð?@7šù‡O?5xŒ,ÙÂ?i!O5ëDí?_éÞiy´?ïÑ!1}ü?}xhí`H?A±Ê#5ui?FçJ!ÅKF?uF6.'U?|ÈÜOé ¼?ï+ð|\ûa?a%"ªçM?r»,ʹü(?}è!ÔN?•Ó%EM«É?ŒbÀôºB*?ï"«Mm"?gå^×
oC?Rn-àñ??ǘ݋žî?ˆ±"œ«?fÈNýÚÜé?ïÆ3È{Ѫ?v¯'O€9Ú?IX¦BÊ?Cì~'Ó"!?y»øÊæ?u"Ýtº?ï\×r`ß?–÷ø˜¯C7?[¨kO˦?e4rb ?'ª–Ž¿Y?–±X¾bE?îv5 î?˜¯ö?q`ê?sFÍ8<el?~*bPkv?¦3ÌF{Jµ?—!X
D¬?îî/'·²?…-%f¼®?\M£zŠ2?U¤ùܓÖï? :à¦Œ?"Q`2§îAGN4FGL J1014.8+2257¿îA˸m÷@K7=áâއÀ9þ†åÀ<XnoId@=!¤W
@Ũ¹?º,Ö¢¹}æ?³yHÁ9ñ"?ò…×Û(@ûRK§HY¿ÊœdzÓÜ¿åfâÂØWE¿é¬u>p~¿ïφ»p"?àË1¡ã•¿ðAGNfsrq2FGL J1014.1+2306OL 220?﹖†§¿?¬Sð}b°?bèáàn?|őÈÖzK?yÀ´ðU?©!H˜?R€í?˜S§ud?hèΕ	Ì?'F½‡=)4?'–·ÎAÆ?"óÂòèÇ(?î3n'>g?˜sÿ¨­á?'ÿQÚ=M¾?P¿T!?£Np+…@¦?'÷?öP¯?ïØÿ'=¡?^7Dç(?J_þ¯†`?FXš^ï?p4yŽ¨ç?Y3(®mÎ?ï îoå?"š_"x^Ü?qkü©d?|—}^GX?~nŠôþ€·?'<ı"Dî?ï
"|Æhô?£$‡Ñs??sÉAt`òV?Œtc^‡w?™É`ÕÃÖ?œ£ü'ðډ?ìùˆ—"¯ö?Ÿ›Ù¢¹¡ù?ž(-ûγ{?"cxãP"Ö?°©¯Ã'ìu?˜hDxZ"Ä?ï`¶N¹ª?…s00H?piçùœ	?r+çŒY%É?áP24•?'EwÞ|ÛAGN4FGL J1014.8-0537¿î'ìxRà@Cúãq*À;û
͹\À<'@eJÝt@¸'r0@=ø{§@K?˹€ôM?¹Ç‡þç|&?íî/ªèv@hÚPCs?íÑóbb˧¿Ù3œÆtÄ¿è@ ìߑ˿Üñ±Þ‰ã™¿ë;<¡Æä«¿ðAGNbcuAT20G J101446-054049?¤¯?zÏÁ¯œj ?^›MÞæý?PÓaWY?†'-AV·r?xäåV3Mí?ï¨Ëï4ß8?yö‹^®¼5?]Ë.ù"ýA?cΣi	°?'žPŒ,B?t}ë8Q¼?ïfCsr=Š?ÆÇ×ôãâ?mÈÃÚw"?r/»ÔáÕ?Žý7ù_‹?|æEÎO0¥?ï5Wà3(n?q8ô>
d?w»ÔÑ2?Xoxæ "j?"fÖOô?o_¡¥v|?ï+%úQ^?èy°Øëã?g¦AÍÄ?XفÐH?—¸Kè4'?Œ"ú·Q÷€?ï6,vDn´?'C#0Õ·Œ?e»…ô>Šc?i¥ގJ?–ƒp«HJ?©'R[7?îße2ÀO?%.вfm?u•uâù¥?u¶©¨?ž®(ÐËã?Œ¯I²0p?í'XË{Ç?Ø7:Â2?ë‹•$2ó?x4ؒ'\E?®t­yeë™?ŒTK›TGAGN4FGL J1014.9-4508?îƒÓ'Ai@"Ùº=À:VR,†À<5'Í»à@	#Îç.M@bE¿ý±q?¹‰M-ZV?¬½™P?ò_äÓSÐ@)Ó)]F'?×ÅUŸ™¸Î?ëàÜ^e;¿äV$ßÞL|¿è°d‰Ø[¿Ö}ÓLKˆ¿ä¼†~3â†AGNbcu3FGL J1015.2-4512PMN J1014-4508?í´	"O
?¦¨=– ƒÒ?r–Ð^û)¬?j˜õC1Wº?±6JWѝù?¥Þnˆ9n
?îŠ׋3?¦‹ÞËöå¯?dXq[¤?o†$̄ÿ·?¦q¡E?¥h…Õ‹p?íÄÈ7w÷š?—ã#ç•ïÏ?ƒán6jÓd?|µ@',é?®» û=Ǎ?–'L•Çâ^?ïFÃîNI1?q‰±Õ‡©Ö?}Ë{"ë?dßõIžÔŸ?iFž'¦k?iz$½.^?êWuˆÔ`¦?¶"@}»Æ?Ž†¸bÔÙ?…Dƒ2g?ÄÉAr;0Ù?µHçÔ©Ô¿?ì58¨Vå"?¿"§ZU¶?}:Õ1SîÂ?ŒÊP'Uý?¼'l]ó?¾.Zþ‰?ê¹ÇÚñS?¦&XøGW‹?•ªU¦$¯?ˆ‰n¸¡Dÿ?Âc™FQaá?¤y=Vî;l?î)¶&Ø?ŒÄ_ÐQ?'äûՔj²?] zwÄ?£ò´Ô!?"+'A֘·AGN4FGL J1015.0+4926¿âN
Bøg@J[9&A³À7!ÄÐoÀ:ùxiž)K@¸>Öªq-?ûþ/Egé?ŠžÔí?¥ç¨ß÷eÁ@WØåó@Yy&1—þ¿¶!x˘Å3¿ÔñëÀ-@¿ÛOqtõ¿Ú"fÝ.ĺ¿àޕÜär¿ØñnØ$ï¤AGNbll3FGL J1015.0+49251H 1013+498?ïç$¬)5¦?`gb¾|Ú?2²õ€37Ù?*ñ­/—æ?f"õU~¢ø?`îB1§?þþUä?…€ÜKa2?]ó€¾÷å?f†0œ…%Q?…ÜÐ*CXA?ƒô§W€n?ïDçKåB?–¶ÍX¤6?mAÞ­Ü?}Šð•É\?™Ï'C[Œ}?•Èü ´qà?ï©(Xl[Q?pP̎Ÿþ«?Nx"—¾a"?6ÆþÙ­I ?ƒÎgÁÚ$T?oÕQJ´Oò?ïÇÛAbT?pôŸÖÊԆ?:+ÔÓ¥Q?4[¨Ë˜?zÓ߯3O?peÇ\ÛÛ+?îÿµõÅ¿g?¡ÅvÉgÆ?oxÌ"å~'?ê%YH;?œ'ÄK;@? 9–?ïá Œ?˜Dh#zºy?fÆ·|£%?xÐBEÿ?™ëŽ5™?—¹ØB:¦ß?ïh«Öe°g?"Åj±8l?VÚLïŸC'?KÇñ!U›?'|à\hå?"'9Ðe›AGN4FGL J1015.6+5553?㓪ú•@HûìÃã?À:`"ՔÀ<®¬&dØ@vÀ7=.	@Óû¶Å$?¼3Øt »Í?¾šNʓb?þÞüz9'@ñµh'?ïõd›‹a¿ÕUšü›¥¿è2ø6#¿åEŸ¶´2¿ïÿv½Ì~É¿Î$¡Š~ɊAGNfsrq3FGL J1016.1+5555TXS 1012+560?ïðJa3\à?PnEŸM¨?L¤~ib-?E҆‡Ä¾?QýÚPÍ?CFZj?ïÎò¥é"?v€ð
˜;Å?RC>ÈÚ{>?`0€/Îo?sõÝb×E¹?pWñïÌ6?ï—#õŸ÷#?~ê¦}Á"?kØhŸ™=t?r
i‹d·?ƒ@èi"¥à?x!D;¢Ò*?ïÜþ§Kš?Q÷Ô¡Ë?eP҇ú`?J¤äû'R?[af–+?A÷ÉÅ
k?ïÞXhy?f·È!Ðþ?dù32‰w?bÇ\éA¤ô?[›\áY+'?Tæ|£…Q?ï^íoÉUc?"îáNÀ?iU×\!°Ö?wjÔÜÿ—?÷—"\P'?Žì#vŸ?ïYŽ×¥ˆ?†01¼‰µU?téq0ŒjR?y¶òk%¨?'¿jAD÷?€-h¿Q?ï~÷Ə`?qÒ»—ô;?'Â1ÿ.±?k:­V_?tºÿ ¬®Ú?`á®#AGN4FGL J1016.0+0512¿ã¸™5_w#@Gƒ*ZFsÀ9Ó¬ºÞŽÀ;ô{/PP@/Ô®Bž
@¿û}º@?§Å#yñw?Œ¥'ÛÃ?ãŠ
jKÎ5@ÇÑb³©e?ï k°RBÿãxQ [ª¡¿æpÒÐòÌ;¿ày7Ó¬¿âAØ}7¿ê'õ¦	êeAGNfsrq3FGL J1016.0+0513TXS 1013+054?ï÷.";¨<?;	dcrW?'õèÆâO?žÝ߯zO?MHsç)3y?7ð‰?Ê­Á?ïå7†mܖ?k8\pó?9™'"¨?E"% °?g§fŠpUV?gm=ZÕiÏ?﮾©jêQ?u='F]´?Vu€Wϯá?CÖ,6/¸
?¥¦ª
¯?t€)˜gü?ïûƒá¨@?+‹›˜ÃÖÅ?ZûÊxˆ>ûäcs»Y??ÐÓЏ!þ?*U21–[?ïòO	ÊÑl?Mµý‡[?0m¡±}S?"Þ½†õ$—?WFƒý?KÞыp?ï",1?¢ìò~õð?L:T±¨o#?Yxšö]?1Z&MWÞ?¢ÖmwŒ/w?ïx¾¬'^?¼òc†?_²ÝjXSH?UMžÌù?Ùù,½}m?€ü&óg?ïôç2?HÈlK"µ	?(â‡"î$?\'iÜã?TÁUˆ7f?FËYÀ—AGN4FGL J1016.4+7703?ނºytF@BmÏÝ"…fÀ<€Ä"(ï
À=§s³VB@!À˜ÐÆ×j?øêܝ$h•?áŸ!"OX?ï2€áü}@	å¨ÃÙD@ÐEìO¿ïÿ.ÿqå¡¿×2ê£whí?ïÔ*pìÒ¿¯ÓÏAé{Ñ¿ÙÕõ?‡ªY¿ïÿùŸé"ÚAGNbcu1RXS J101647.6+770239?î"®çų?À™#<›è?¢,%Ï|½[?¶Ö«rßñm?š#^‰58ë?±³¿Ãï
?î®rÅ«Š?¦ÆªK}ç?'=;P·HC?ªò_í÷?˜ôkù؆…?–=HÁ×ÿš?ìQFbÔ¥M?§Ëe lc?«_‰
;o?¡êÕUúŒ?¯‹üI¨o¿? §ŸÝ#´?î–Ë}¹¶'?Ž@ï…õ¨?'Ûª¨c°?ÛÝõ¬?›J噆Ö?‡ ØÁçZ?îš$šFÆ?±ñº›É~÷?˜'¾7'ü7?ªöqj^?<?"<=.Dó
?¦Ž¾'å?ì2Ê°gç?½¹á"DM?¨¬bÂ>"À?´ƒÆ®ˆ0?²ÀHg?®…à+Ë?ë;Œ°`Ê?¬[‡8Žª?¨ÓÆOÕâ? r#¥Iñ©?º5¦ç>?¦Î{öáíG?ëÞ¡'évH?­y"3Ur?¡·Œvsä?›ƒw•Ïå?¸/i#TúË?©Y‹ñíAGN4FGL J1016.5-2650?ÕY†^m7@8oawêiÀ;2üÁ‡À<¥D@¡°¿@ ýçP[¸
?ÿ'6¾ØîC?Ôï˜ß_vˆ?ζ`dCÌ^?õr-å˜î?ý:¥¸‹Í(?î'ØÚø¿ïøžwNëö?ïÿ¡Ö~ý6¿Å¾´Ü?,¿ìè=Öû#ø?»¯d9ÕåAGNbcu3FGL J1016.9-2653NVSS J101634-265057?îÍjKÎ4¬?•âvñè©ç?~1Aҙ{£?s®bÑøÚï?žÆfÛ=Ÿ?"½
FýV?ïŒúJ›?›ç¬Ûô¢?ƒMš¹fò?ˆï…ōyŒ?–±
Š®«?"¯E«,?íÕ[ÍÂQZ? !
›M)?‡PQäêžñ?…eLÇ7V?¬Ö.¨èt§?žد¡FK?í
`§HÉ?— r5Xz¶?‰í7Yv?yævû×¹?´WW†4ô?•Ìì<Û|?íOw›õ?¬
á0-±?‹0¢ø!–&?€×.¬dD?²/¤$Z?ªžûHÚ;*?íMÙU'y©?±¯6FG"ç?•òÿÃB€?œ±òz7j?°J¸•E<™?¬$µÍÔJ?ì\"$d…³?¤|m‹7›?ŽÔ®éCZ?ˆqÒÖCû?¹DXýû¡?¢Ê9¶ºN¶?èPE à9*?±êC)|?›ôòß+?—Ù½îÇû?Ë\lùŽ²ò?±ŽƒˆÅ'ÅAGN4FGL J1017.3+5204¿ÛÏj湚@Iü¦\ö{À;†ì"øø¥À=š‹1!
@ ¦ß¢ú@?úpŽX÷ˆ?ÓCâb¶-¤?ÔÄO»)6Z?ûj÷	·8ç?ù&¹Ã_¿ßW7õ9Ó?á£&`;ÿà¿°Xߕ&mR¿Öƒb¯É¿à¨Ž"'Ùd¿éҜŸÞW9AGNbcu7C 1013+5217?ï£ß'ÄŠ«?yo1躦ö?[6pJ-L?JvL"©ó?ƒ¡MTµü‰?w¹!=ú í?ï_î:
?ŠOî!R­?qò7öªt?u0\"Ñï?Ah|¬~?ƒ'ZŽ¡*ù?îÁÌ+â?–©ÇgœÂ$?xÛ­Ó¨?wbQA…Ã8? ÇÝ{{z?•
eÂN/?îŽOÛ×Ï?€¿rªNî?"åg:†?ž?rŠ!Ééo?¥$gaÇF?{ÖIA¢?»?ïbN>ÚäÆ?ˆÃúñ`3?ihÎvBÄ?Y_ß-|Q?‰5'¼øè?‡V•oÈü?íüò é<?¦»^†q³?ˆíÛ ˆÈ?Œ´Àø"b?ª5[¹®?£!jïCq?íÔÈäWOj?¢8±=Îbf?'m¥‰4Ç0?€,Ò6:D
?®TJJ ? ÇÃ?¿æ?ëVÂPêK?˜¸ôË¡?ŸÛ|N@f?ˆÇ/»Ϭ?»j×ÂÒ¬?–ÉïñÁ®AGN4FGL J1017.4+2538?äÙ÷5^º(@KÏ\WìÀ;Î²€À<ʴĘJå@#mükJü©?ñxá'ͤc?Ù~íEé]?Úu$²?@Áù£Åm@¬3ÁM'°?ï»U
ôOÉ¿ïæòåˆ[¿ïÿè«î0?ïÿülò¿ßÙ%ÀÙÏj?Þ"ø!å-AGNbcuNVSS J101724+253955?ïN?‰‹b?£—ÓÅD?U®³¤¸&½?\'fwj/?"álÔÛO?¢…qêb?ïpÔ³˜j½?'Ó«ØVú?o–ï<ï?z²Þùòã?Œ-nõ—v?Œ»UR®'å?í³"!j?¢ð¨Ã.ô?oæx³ÝŸþ?r8øwQ‡?±d«0õà$?¡¾½çíêž?îß$P¨ ?'…í˜ù?hºº?hJqÎY€Ù? 'Â|«'?ŒàÔNrë	?ïTÚX.Gð?"®ë"U·-?bK'Ò½z?fıŒµÉ'?"BÇ<úc?"UŒð%?î©3B?©b"gä0e?w@\fà@?†Áñ˜jÄ?¢Œ‡ßÉ-û?¦í¼'8L?ìº3ᦰ?¦J?r9a?räºzrál?y:`‰ç¤±?¹Q/yi?¥ó!é<w³?ëÆMOF»?±'p€m?‡IIcåòR?Ì©‡Ã?¾älYM+à?°µTN˜ƒAGN4FGL J1017.8+0715¿Ôïm#¹™@HGÐ|"µÝÀ:´ÿK¥À<N°ªWVÿ@·ê)))@ÎɟâÚ?ÉIO>ׁ1?¹þ_ýý­|?ì>m=ðüW@
QÃu‹~?ïûŒž"#¿ç?*¸:o¿èÒ¤Uµ>¿èiʞõ#¿ïô£
[£•¿ãú'®š²žAGNbcuGB6 J1018+0715?ïóû/¿=÷?YDýÄ¿Ã?4-*Ö<Ûj?0¼÷
ÞP?RþVF"ù?V'½jμÑ?ï­Çl_¦?€yû""á?^Ò6o?d¬mæ‹?€µ²¥Á\?zm+­PY?ïŸçæG‹õ?yŒmöKuó?`$,*‰y?]û˜-.—?ƒüûfÚ}?wã@ݺã›?ïœ6ûGg%?aûþUÙ?n:|Þæë]?PûL¡8v?c¡úŒÌ?^Ïêô.	?ïê̤UVÁ?`êçô{?=µ?ŽZ‹?5W|'Édï?a|´†'?^ºm—ç¡'?îýÝw%6¬?«½ln©†?p$1wA6?|ّÆWbö?œ;D¹=Yð?ªêa¦©œ?ïL~{[$?ƒï¡RësM?n¯-:,ïö?q±¬QÄÑ?'šJå­}?D"Ù½2g?î°<J€y/?ƒrF;÷¥?ˆÍÌ¥UQ¦?qˆAá®|œ?'^ýÿY?ˆ1g®AGN4FGL J1018.1+1905¿ç"G¸{\@KÉÙÓEÀ:xàU¬ÛÀ<"eByø@FOo©Ü@˜0LÎæ?¹F½S³{¿ d¬Á®Ox?æîÆؤ@	rmœ™ì¿Ù·
bZé¿åçZíŒ_õ¿áá›@bƟ¿åP—&ø'M¿Ëªø;»lþ¿áTHÏAGNbll3FGL J1018.1+1904NVSS J101808+190614?ïã¶G>Þ?gJ³ù³]?AØ#ðåU™?E1€'ó?gÓ¯®p£§?bá"Âg6"?ïÝsˆ¸Ë¹?n38†ð!Î?>R܂N1?F-XÚÑOˆ?nÂÌè.?kDZ¥ûk3?ï¬Ãªº(Z?qíóÅ«a•?Q¤zèc_+?SëD•Þ߁?'š…ïš	ˆ?qŸ=13¶?ïϟpÚCê?U£†Ú©ô?AÔ¡¦ò#?(ãÑ¿æ=I?uõ³kìÓù?U¡ÿB
©Œ?ï¹IH"?t‰Ÿ©q?RZnŒ(Û?Eš"'æú?z¿¶£½w?ràÙt}ä?¥_(?'`¾4BL¸?P;Ö6_Ç?X¥p%x¨½?–¡'ê?'Ôivë?ïeyìL'K?€óÓÕµ=·?Zª5Ö,Ø?X½Üj‰Á¡?'¦;?Ø?€~¿øwÑ@?ïWáV$W?x%.D'W0?[۔Lº?MPâüß?"Fý"gq?xª=ñ<AGN4FGL J1018.3-3124¿ÅN?ö]@5ÕW2À9´¸ÙÐÁÀ;òŒVºø@zõ }ùÖ@°1;nÉ?ª
¹|
¿?®ƒ
¶è4@	Wɱ@iDû‡ H¿ºNnxƿᦕ€…K"¿è¸Ëž#—	¿ç×"'$€¿ì3bƒþ¿ïÿò(¦è7AGNfsrq3FGL J1018.4-3119PKS 1016-311?ïÅS4–›Ê?q—ópŠ_ ?q$¿'PŸ?hÙêøˆ?gªý}e"?c-aÜl¾¡?ïƃe?|
¥z—Xž?Y€›†Ü»?gØ]Åõ"?v"—<î+?uEY_ô…™?Ô6?';Öð?q¬zGõÝ?uëe¢F;?ƒÛVǝ?}tHÛrÎE?ï؍˜.Š'?QñÂ&_øÿ?\ªýöH?B?M¿Óñ?i*WÛ[?Hö¹ïîdÃ?ï™\§Ë¶?€³.D	L?~¥Jö?wS 
ÑÞ?uY¬žÍî²?q‡Ž²¾aX?ïkœ8Zdz?•¸ž¸)Œ?jd*pǶ?"C/WÖ?Ž"˜ê!ec?'Dz9V@‡?ïSÁ²Œ?Û±šRà?vZtÆ£Ã?z}µj3¾?ÊϨ'ˆ?ˆˆ?D²Ž=?ï‰$åÆ?s´U¬_¼û?wo<%´Á?c±¾I>qÝ?'`tl^?j~ïnO^AGN4FGL J1018.4+3540?ïýebÁ|@L=
à"S.À9ÌQþ'BÀ<i­1üÒN@ðÇP6#S@G³zì/i?µÕRWeÂ}?»8­ªÑ$?ÿ»ê&z@±~Rû¿ËžM]€ä—¿áݑ`eŒ¿è« —ºœI¿æ@>-b9¿ïWàyQû¿ï•ÂH"AGNfsrq3FGL J1018.3+3542B2 1015+35B?ïÓ™wq?¥ˆda*F¸?16:û¹‡?'"¹@þdC?ufÏy›¾Š?¥ŠîaEl?ïÓ£vùAÜ?t±Mï¼ÛÒ?LO¾omÿ?\ÔȪåW™?r¤aÉö	?p2cñì<ç?ïz!I¯T?Ž‰Ð¬]õ?CnÛ™?ˆÈßʃÛè?€4?{Ù¨È?{¯òò‰s~?ïò]Ù•?@d°|›Sä?L˜Ó_|_?5֍XDê?IòíÄNY?2Œ}Š>é?ïóo¶Ãs?[̪33úÕ?>}߶9l?8À¬Ð¹5?Qš´ÄfЅ?Z=Ê3P?ï¸#"Ò?‹}¥È&ù?^fñ€Õ5N?lÖgƒY€?ŒEÜòi&?‡´l%±û?ïif˜æ@f?ˆMªlu€'?wùªú2Â:?؏8À?‰©"TUE@?€k•C®^'?ï×eÏè‹?`dUOŸÈÛ?f'h»/â`?Wh"e˜£4?bnj_Œ?Q"Ï}´¿AGN4FGL J1018.4+0528¿ÜÈÙo"Úº@GÕËeè'À:,ßØBKÕÀ<öó4@O-\¯ƒ@uð¥)?ÂN…7x'?¸¨*ÕÁ"?öš۸ù@†ü®'ÎI¿î¡¢7_é?ïö€Z-s¿ä
Ÿ¥Í/¿åÓsD›:"¿áŒ	XnV¿ï¬¿EûŒÔAGNfsrq3FGL J1018.5+0530TXS 1015+057?ïéԔŽº:?W›ñFÙu(?:`TgMG?*0'Y
ˆœ?bꟊ»*œ?V"óß.?ïÙå"øRÀ?pÿ%È+?DpXšií{?M—s:š?p*\é'?k
wÁBV?ˆ™õ"?'J+I¾;?c"'ã~ýÒ?h ¿K"‹´?‰½$wà?€-V²	Ä!?ïsý[ñÿr?jP¢¦ÓÔ×?m'L
(?PqK³úm?‹œUö&™d?håöCZŸ?ïݔ´mä?_«øŽ–	?PI+‹¿R?GÁd?Õr'?jGgÉ5??[Žy'o0?ï"lË:Â?Œ×ÁŽÀ
?VÊÅvŒ?`¾¸Æ[G½?Œ‹\è?ŠÞÐâ.~†?ï є1г?C>+$j?qtÿ"¹?r&gªŒ%?—žê#eX÷?‹fE'~)?î'q`?†'w¸ßŠ3?ƒ•ˆ>¿*?m'm?¢óâh?…­k}§vAGN4FGL J1018.8+5913?éM:ì@HIÚßµÝÀ:›&Š®DÀ<Ì_‹€Ò"@¥¿â®‹?ÿ•a%´Å?ÀòBÒãg?¾o/êÖ?ÿk/=Û,â@{Ùs¤<‹¿Êk¯¦vKâ?ì	ÒÄ]"¿âvIh(ÞF¿à©RtA}¿ßˆn ¿ïÿþBe«+AGNbll3FGL J1018.8+5913TXS 1015+594?ï䧽|Uo?gl<Õþë?V`ŽJóƒ?Sªä?`'ûf§²?dy¦EÐÍ?ïÂAÒnˆ…?|Bìý'Š?X,ß6Z?b—´D?xÔRsÕ?tíëlÖ[,?ÿ}?oìyÉÿ@?b	™Ž)J?egcK\ÕX?…'ÌdL?gþ:Ž§é?ï`)…Öý?kúo09Ü?†q"g·'€?f‰Gsý?"
>YñP?aˆæ'˜Ÿ?ï½(Àú—Ç?vç6H§Ó?rÝC­øÍç?rEöpÀu'?m·¨ÄÆ?b»yñd-?ï6šŽ|?–øgƒêâ?pŽ!wKh?y}Ò?‡½??•	6¼R÷·?'E#Üø?ï<—J‰æô?~@9€Öß?p,)²3¡÷?pü¶¸y?"bIpö?xIÐTÕé?Ùû4?†ojPh¾©?™¨œ›ö?'Î|>.?•A7áKg?y–qUᓘAGN4FGL J1018.9+1043¿è?Vx÷Qu@IMæ`ɊÀ:ÆIéXÎÀ<f,§þ·+@Éáš9R@·S´Eí?ÑĬ{*C?½è""¨¿?én
ŸOæó@—©Tw¦¿äÔ§Awï{¿èôúþ¹Xý¿èú³$…‡¿ìÛÄanYû¿ð?ïÿ—ŸïI$AGNbcuSDSS J101857.97+103625.6?ïߐçCp˜?h7.ñ'E¤?W°B§i@Ù?UŠ©1×.v?d–÷v™7h?bÑѽ!1?ïi®Â3›?"Ö$r!ÆÔ?qÅðvâk?}«úRŸ?ìsáB2?Œì&Õÿp?îÀô¶dšM?"¦ô	ÍjI?~*ÿçX?P^½Ô¥? +Tœ®YÂ?'*ý¿òW?ïÊ_»Ù5?a2Òȸ4?XÿªIH?Eѹ\8?tŠ
¡ß|?[¤zfÍ?ïÀˆ®ÃU?ˆŸ8°nÉí?lTÐ	jÔ_?pé°Ôáú?qtS†\Gv?…sí~]?íâaÞäžÈ?¸£-ðt?"ö"¬"?'Gx¶5?¬¹¡ðÏw?·Tjƒ"Í?íš&I"Û?©-ÜWI?ˆuHV†?"ÚP-öÑ?°,­=R€\?œ	󍚡›?ïFfÀr?"r©;c9?pù&§ö‡é?elHŽY ?'ôóI´°?'GЯ•?AGN4FGL J1019.7+6321¿Õ®çé!°ï@G % …²À:h!È`À<'ž1Ún@‡-nÎõ?ÿ
ýÌ=[?¼]Ú{·?ÉgÒa·*#@؎6F@"‹½¸Þ?îísk1§B¿Í¶†9j"Ù¿ÞMdºã¿áŸ°9F¿æ˜f^ꖿðAGNbll3FGL J1020.0+6323GB6 J1019+6319?ïèù!Ù2{?YDþ†?Zª°‹*B'?R3\È0Çz?Scçgá?F¬ÁAÍh?ïÄ7èN³l?{0ÅwEjC?V†­õÄWP?`öš®q?xB`W¬?t±ü¤oMM?ïcÖ ³~È?ŒšG|[ê8?"¡€Œ»p?‡úõ\Áš?'h÷>&2š?{
š˜Ø4?ïv9JÐ*?dÍiQÀ£‡?x!g7(›?V~Ñ6¢¬?†aÇxž?]—PÓÃf?ïÍ(GóQ?nŽSÎP?o'¾WÄ?gy$< ôE?c¯úÖ3̋?XP
.Ú}?ï=b"¨KÂ?"GÛ©?mÃ3@&:A?tˆ;a£³¢?"›FýFe‹?'
(ºò?î IV`3ò?šâ0Ž';?ÐʒÂ?—ÑÈÎ%ï?ÔÒÍÇè?'zØ-?î À !P»?'=dz~H?Œ4¥êƒî—?qàÄÐMæ‹?Í™l‡U?|ZÃøÂ8êAGN4FGL J1019.7+0511?Ã0Рt‡Å@Gâك"t—À:áüjIJÀ<pšäó4@@ Œ£jRÚ?þú¢
¢?ËÌÆÐ&?¶IÏAq9~?íM	""}Ì@
!N§-¿Ø©Ý´{/¿æÀaïß Œ?¡x­™W¿ÖÞ¾fØ|-¿Ú<XüŸ£¿ê<þޗÐlAGNbcuNVSS J101948+051327?ïôÝ$]ØM?B!ômã¿? ìÔ ²?)C_z/M?T[¨",P?AØsÜ?ïÞìë-é{?jàt¸ÑO¹?9½7ÒüO?C̝þðÕ_?mÛmÙ]8?hö-úÕ@?ï ¶Z'ü?{†(nû2«?L
áÖ`?6ZËÞÈ[?†¹X"ž?{U:í+Yý?ï¨Öí{ݶ?`AXbªä?B³Èlª–A?([Œi?"ŸUåh?`p|ö
ù?ïéLô"*ß?W&'G׆?)˜zˆqK? zÒSt"p?eƒ"8oA?Uè†ò7}?ï'yìníb?‰"žq´g?PRR†(YV?XՂ4l~?‰—:–?L:?ˆ'™V1ß?ï1W[0¨>?‰Ì©%"°K?UþìWH:¨?Iû–oš]œ?˜u%Ñ2Ӌ?‰Y¾d¦?ï
ë‡ç¯@?~Á,´‹Z?TdEøþF&?DSØÒçŠ?\J«5R'?~s"á tAGN4FGL J1020.7-3920¿î&V—w'˜@-¥ê«%)À:õgXÔ­lÀ<"UàÝ%
@ dæÃC?þ*™Eå½?Ê÷ JÂÌ?½Ù!™Ø®­?ôä$7í'@ÜÛNšÂ¹¿ïÜ>Å7­?ïâÉ¾²¿àِ"Š¼¿ÍOÿ‡4<H¿æEz=]Ùz¿ä¥ ¸ò¥AGNbcu2MASS J10203893-3920563?ïƒ8(\âÑ?'	sÇ÷?8²òï	%?${øŸêµ?Žq\Äæ?'›ìÉÜ? Y«‡?"FËDý*!?\'.7?›?cdíªdÛ?ƒ"Dš`?"Ðfc?ï_cQLè?SÖ43G-?aùíþM?O~‡ô×ò›?'ÐððXó*?€RÏÕp­?îÝê‰ûÜ?vœr£ߖ?€3Ó×W?]''¦2gZ?œb²óXÑ?tC"ä\]?ï3}G9·?š<j]yªQ?Dð²f˜ž?5(à¿Ž?˜æŠÊ/ã?š-
ŽÊÒ?îç.'æ¿?Ÿ¿JJi½?pùº°±^j?|q·š7?žÛÁ¾Ú•?œHˆÎ†?îËM´qiØ?ÏsÅ?l:dˆi&?^ñ€Çvݾ?¡‡~sQå?Ž‡eôØWæ?íB©Š}r?'"–Q8ø\?²×Âh?x|¦ƒm£?±Îæ+¾UÙ?(3RÒnAGN4FGL J1021.1+1626¿ã€Ñ9v¡Ð@JÕQa£ÊÀ;cüÈ=À<ÇG&/>²@ Ô±šA_F?ýàA8¯sö?Ó? ^¯¸À?¥Ïƒºþ?Ëáºö¶€@nÊ£|ÇQ¿ïÿÇ*Ì\e?ïÿ<‹¡‰R¿æ‡9zu$¿Ã¢ÓÔþÊv¿å­å˜îy¿Õ¯=oÍAGNbllSDSS J102100.35+162554.0?ïçà×p¿±?ƒÃë¬%Ø@?0uQ¾…¾*?)-5''Üê?f~"íž?ƒ¬s%½…?ï×CžÃÙ?pitD>Ù
?E^#/Õß×?NKtÌö]S?qЙ­M?l<XS†Ã?ï]vÚ)?"2;MËEQ?_"e"Û¢?`{?Ă?'Xp?TÀ?ƒõ@é:$ï?ïAz–?kӘ=Úô0?i÷j÷?O@5f5ú?‰ÁþÚ?iæ0ué'?ïÝ}qùJ7?ax>W5f?<"ÚœŽ"(?0_$ö@?nðËTiÉ?`§Ã›#F&?ïqßÏÅ
ó?Žü2›&Å8?X-ãÃíI?`"x€^Ä?A'Ֆ{Ö?F½Qû7~?îñr¦´Ø?Œo)³¡[?dñ~ö;ÄD?aÁ\Äå—[?Ÿ33)~?‹Õ)S»?î¶*<¥³ê?†û½uøÇÖ?xW$¤Ü:?i,+šC«?¡'wŸö_U?†‡E"¨îAGN4FGL J1021.4+8021¿Ôi»ý¾ÿ|@AM˜ˆøbÀ:W‡¦RÀ<˜ƒÛÂ3@"¸_˜@vWu1ÛD?»î›~¡Â?ÅӊV/·@~ɄBð@?üo5JÁå¿Ú¶ÇÝyÃ:¿ßWsÄÈÇZ¿ãd.]‹vk¿ãºPþöſ×øz?Ϟîm0…AGNbcu3FGL J1021.8+8023NVSS J102201+802350?íÄÇQ°Y?¢à}lˆ¤?—»GϺw?"´úþï?§Õý>'è??×ÔgEÀ?émÀÂ?Ç)·¥Y|"?ÂV|—÷?ÂßËÏn4?³Íê¨+·ý?¬@Ÿ<Ò¶t?ìóŽ¹ÛrF?¡¯ì÷w‹Ì?¦Y¸Ú±Ï·?™U¶MõÐ?ªm["'oð?—É"Ö‰§?í=;Ã-Dd?'©ûÅss?¬‡?Àà?&;Z?ŸJ–hU¸?|jÃ29L?éyQc†w?¸(†"Ú¥œ?¶¾|ýׇ?­/œM5	?¾¶d«{C?²6J†¢K8?ä$JǛ×Ú?ÎTæÐó¼¿?Ì؍Ú?ÊxªG6\?ÃOº	s¿?»rlïHo?ê¾4â?®H‹øÛÄC?·löƗêÈ?¥;äsv^?¸5'
¦S?£Zù@#?è°Ôאӫ?«]TßtR	?že.5¦?¦©ýïùZq?µ<ŽåVHœ?™ ]ò¾<ÖAGN4FGL J1021.9+5123?¨O\šÆÑq@Jt×I''?À;҃9LÀ=Š'¥aN@ƒ{³žÇ?õ¢Œ¢:R?擥cÒ7p?ä³øà¦ôK@¸d"@úø´‡0¶?徚À
F«¿âs1fªY¿ÞçÂòXx¿Î û;;¿êFJ'Û¿ïâ~
ÇÚAGNbllMS 1019.0+5139?ïosùª"?‹uë¥?|Q•­Ç¾?xÐ÷ó¤Ïn?…útÄ°Æ?µ>!¹J?ï=%_Šÿù?•Q`ü·N ?uÿ–PA?{Îøëø'Ñ?'ûTPË?Ïζ'4?íæÄÒy×T?që4?Žç³å~?‹Ñ掫.6?©ïxè+õh?˜¨¤…x'ï?îŠÖ†Øø?"¢(æ2?€Ã}KbÝx?u,ÄÐÈ8¢?£!¾²&+?^Y#Iå?îМr}t?—ZH–—"?'Àݝ'ñÝ?Œó +k)?"+"µ'˜?ŠÆ`—²s6?íÞ÷ q5^?©sÄí·&h?Šå¿þV^f?"&Þü‰°?«Wú2ùŒ?¤KʝŒ\3?ìÀÉ]Îߙ?¤môrØj?–Uå/‡;¥?O¶Å¦G?´d;ŧ4O?¡¤ÈS™Ä³?ìé¿Líª¤?žR£4µÛ?€VÓäkƒ?†‡6ââ…=?¶§+:†Ý¬?œc x°AGN4FGL J1022.4-4231?è 06©ŠR@(¶Žæ¸0^À:\a5¤ý{À<^~ø-£§@4Ö ˆŒ@ª"£hO?ÀºIýÏùþ?µÏ?Š?öFB‰èK®?þ¤ŸÔò
I¿ÜÅÄDèè6¿Øä2"Œ—(¿äU.enâ¿á=u×H¿â°T[¡çF¿çYº¼)›AGNbll3FGL J1022.3-4234PMN J1022-4232?ïn£TêyA?"ÁŽ&0-?aR¶'¼)?Tx¼g—ng?>—¶¿?'•˜B(†î?îênj¹(Í?Ÿ`ì6ÆüÙ?q0sÅd¶?q r5"·?žfèÝj"?ýÃcðÕ?ï,ó^îB?'?AñbÚ?p´éf?féVâºÖ?–[Úªj?€v%ʬ7?î³åŽuà=?t…›€éM?…NÙý˜äÁ?`"Ãvvѱ?žÛá5ç!ö?rpŽÁwüµ?îŽY¯ž¾?—£X!c¯?xüLsÎg?mŽ—iñe?¤%~Á[g?•nÉƹáƒ?ìÖEc}?¶¾»xwÇ?ŽT&"˜9?™Q'(mÂ?µƒNÃK]?´c3jHoÇ?îM}K…?–Y;PP3ü?ʍ¡K'9?s"1E2gC?ªÝTՅ?"Ëp	p?ìŽ5Н?'>ž'SÛ3?›,ðžÅÓ?ÝÂ?Œ|5?´ÃØ®¢?-½Ø‡#AGN4FGL J1022.7-0112?ïhžH™»—@F08⟜éÀ9˜püÀ<Sq@€bÐãå?þY·+zØ?²ã2½—{?¥(+Ã'\?ó{–^{¶Z@ôœ"µâ{¿äÓF=üåÄ¿á¹\þØ<¿Þ2½—z°¿Úv7_ÞO¿à‹aÝ냿ßä€]2‹AGNbll3FGL J1022.8-0113RX J1022.7-0112?ïâÓ|òÍp?SÂØ•|á?Ciä×À=-?2I‰³:»Ù?hR	è*.#?QÌH#J~õ?ïÎN‹I?ua².š)?MÇ~¢jb‹?Ua«&˜õÍ?u 
EöŸÓ?qåÓmH­l?ïv `œ?xÇBßw™?e=§‹	?`çË4(?(™z…šC?uë'¢Ã?ï hL3y?s"•`4Ø)?x6xO'?Xúî?•í)í?p"K · 
??±N?i¯³½ÙS<?XOVÊæ?GþZd¨?x§pñÎ?fϹx™ˆ?ïM¬61óÌ?½Ÿ…ÑB?e~r›Û¤?oå`í­¤]?"šªã.h<?6ñQ8…?îé<löV?‡³Æ¬ÒO{?tÄðO	?n[-º+Â?§pd™ª?"é~=°€4?íììí  Ô?Y|Ú,m?‹Ñ¡n¥?râÃò;?ª<Èê1e?ŠmL$>ûHAGN4FGL J1023.1+3949?Æÿ&ˆ¢Gà@Lo1½èÀ8ßÉ#ÊàdÀ<"àæ_E
@ŒÊ(W¸@ùÅS[È?¤L/¿œsÐ?»'Æ€FP5@ä­Ýô<}@ü9§¿Ì†ùXñÞª¿áíÁ9ÓÁ¿ä'ÙaÏ©¿éDåw¾}¿æV†''>¿ïÿúŒ—ÓAGNfsrq3FGL J1023.1+39524C +40.25?ïï:™j0?S'Ëj'Åå?CÊÛ±1£C??(.\݉?W¥^ó¥.›?Oøme¬?ïنzi8å?q:6q¨ý?DM#i•ùø?O&/n?p³jl7
?mYiú¬d?ïrÿÍfa?ŒGœÌ¨?z¿—²û?ƒúd{zÙ?†4lvÔP?"â}«Tì'?ïþxC2¯«?6íÓ@_¢?^õ«>õrߞ
è5?#7¶¨jHÙ?hRí¿V?ïܙv¼¨p?lƼÓ^?BñÓÈ梅?>õnE0^?nªó›¦?jîDvz?ïR:+í;?Œ\¬¯=H?W\0¨¢t¬?sÌåe¤?ˆÿën^¾Ž?‰öÏXÈb?ï-4…PP?'ËC{Ik?z]«î
(0?ƒ	þ…{?"ÂT¯Rë?Ž¼â·të?ïü;zT"è?1h7²!0?ôѲÑê?ŠçQà¯W?8&úQ¼.*?.— Û¿ÙÜAGN4FGL J1023.2+2859?ï9U¯	@L²82vtÑÀ:ªÐ»nÖwÀ<Œdý±@xšô¬·@uX'?ÏÕ£5#Î;?Ï?/*ee?þˆýՃU@™½Uá]þ¿Ú0œ_ǐοÝ&‹º³Å•¿åâ,m®"¿í½mHضæ¿ÚØïþ¯¿ðAGNfsrqTXS 1020+292?ïÁÙB•À‹?síAt²	?`·*t­Üß?\Ý£f¦m?v·É]<(H?pIÁZùÙÊ?ïÁŃòT?yIûòVu?Tùªê¼"P?c3ÃdÛ
?yÞÓM!+?sfo—ã¥?îʋ#µî?'l¥T>Ä×?…½
Ž®–ò?ƒ‰Â:êc?›Ð>–ú¿?Šø†•Ú?ï¸ð½ÓñÀ?_î3TaE[?e**,Å¢?P[ÛáM?xò‹ìf~è?W§%µ§ ?ïfí:35?Ž°
¦"˜?iCç _žÞ?cù–/0?…\Ƌ‡?Œ5ÛŠØ?ï2†:QP?"ÃøÕίú?i[µð&Ã?r5Ò!¾?–ƒÂq"?'FÐç0O?íZ$=™`?žê´n{?˜tw.c÷?'\Â+nè?®#€'Öi«?–ÈúO¬?ï;YF\©?~äsdØ?xµ{Ž?mûü%°Ñ?'gxHáÒ5?yLí½1øAGN4FGL J1023.8+3002¿â\8Ì5‰@LÍ®>lLYÀ;)€z䢬À<µb+nBÔ@!7¡¬ãx?ý´òd/U?Ç}ÖZHŒ?n­àMˆ?·¸Ñî×@€Qû,Ý?ëÔD$òþ¿ç³VÚh¶¿æg¾U:Å¿ÒÙ~ —O<¿Ô¢ÃäÆ¿¿à§".ÍüAGNbll3FGL J1023.7+3000RX J1023.6+3001?ïÒl,Â{?n©­IÒ ?8êR­‡?2x7Òç??uI«E¾r?m%1hÞàÓ?ïÄ{—G|8?y¬ñ'…ƒ?FAàDUÉÑ?L²ox³é?zùøW~¼Õ?xVųËü?ï{þºÁÄ?{äĽð,?Pú½×ٞ¬?:^9váR?hžëa9?{«©¶ýŸ?ï§AÅÈ Á?f9ÿ‹'V?K±ô]x>Ë?2"2|€?"toXzØ?f~µ¥UE?ï—].%ϕ?ÙµáÌT×?CäžÁPN?5cƒÆ)¦?ˆêj•À´?‰Â‹Q>£?ïH°ÀҘ"?­¸Êø'j¯?QTµcú{\?Weo¿¯?•Ôœ'úÐ?­¸M^¹'	?îۜƒƒØ'?ŽüÛ膂4?VRAtI=?Gƒ¾Iøó?¡"¥½(ô?Ž»ÕL°Ú>?îĺW5?‡((Œ<ï?eVµcbœ¡?UôÛ,ã˜?¢i	œ¨ì?‡e±Ã6?AGN4FGL J1023.8-4335?ï¾nš^ÝÓ@'3ó.ZÀ9"Üõ)À;¸•Ew–@ 
½Ál‡?ù¬gíO#T?°9?硏\?¼ßyLȼ@ º}>ð@¥['¡'­?ï÷=Bÿ¿‹â꬗ß@¿Í/?ɸ3¿×•)<ºEŒ¿×úžAI!¿ÜÞ&¼W^·AGNbll3FGL J1023.9-4335RX J1023.9-4336?ïÓŸß?&?u0ÛÝéW?Fòþò%z?DÎ'U2š?s¯'¹·'t?s…»"
µÝ?ïrG̃Œù?˜S˜[ë‰?[‹«X¬"?gÙË¢{ ¥?ü—lxE?—ˆL«"q¢?ï¢èÞâ_?'Àžè¤Hé?tÈâÒ[£³?}4ŒŒˆÂ?šyj5d!#?Ê7¹ÏP?îP§Vù¶?"à,búð"?w™(u©?YûJBª-À?¨e?½I?ƒÁPö?¾?ïŒsIp.?‹nMô&Cf?WMÂ>e?U‡É ºûŠ?Šjê<pà?‰ÚBgi×Æ?îXºÓóT?°Š€Ø´ù?~‡'$ë?š÷	*à?¦±áÑü‰?­êÇ±û}?î›2µ×4Q?šï•Z·à?y)û´b‹?'E¦?£'•)Ï/ž?˜?­o-m?ìY%ÿ º"?ž+$²A$E?…ÉæÙâ`½?rI\ÚgeM?º}"-¹Í?ƒÚ?§	ðAGN4FGL J1023.9-3236?ï÷ø5A'@4½Þß)À9høH{™ÔÀ<h;R¼@ÕÈ<DSí@Yú—á2µ?°¡ŸL‹ôÀ?¼ODyׇ@ "Ú@¬Ûù Ý¿Óå•ñnlÅ¿âã}_*Þ¿ç‹1÷ÉЙ¿å¨âaßn¿è¤Pwؕ¿ïÿ܎᯳AGNfsrq3FGL J1024.1-3232PKS 1021-323?î…7ÉK?˼Ehóg?=À?nh@?bÕîhŽÃ×?­ü,:³_?˽ØÑp~ ?ïç_:««?kÑÁ/‹
??!ê÷Ø{é?PÏþ0û&#?d¼‡Áf"…?fÅÕ'´û?ï¢Á!.4,?}û^Üâu'?fX‹ãs?rbÐVC?Ìïç–î?vC#åé '?ïùê ®qÿ?*{9i?Š? ¯üþ'Ê?ÊÕÃj»?DP¿êžÉ?'¤†_DÚ?îTÔ:?¤8öc›j?A°‰±U^?>Ä(ó'Bb?~'­²Lc?¤< ì¯wD?ï±sð4'q?…&PùL¥?T¾Çú ²¢?f/ÝX'B{?*éS9e?ƒ!«,Þ?D?ïbȂ÷Qí?ƒ|U.9?o3Ib ?p/H89~?7b¡?€1Æ[›?ï禎Œº8?L‹ç°1«ñ?7\<¤E¤
?)˜²W~ô9?ZÕÉÄY^µ?I(X± <þAGN4FGL J1024.8+2332¿î8Œ¨3T/@Lf/¾3¬ÖÀ:Jº))À<'ÜÜåHÅ@ex?V×þ@Ë\ŠD'?¹ÁHà®ø?z™™øÛ?¿¹:^J¹@0g…JW<¿žóÂbe¦¿çy€‰þ#¿â˜ ˆ5Ä¿çJ†¡oPñ¿è_ÊÀØøª¿ç_·¼]êAGNbll3FGL J1025.1+2333MG2 J102456+2332?ïÎ{øbÁ…?nÿúèa#?UyÜ]a ¬?G}&¨Ö¤?scŒšj=x?l;•ï¡Q4?ïÉÝ÷S?yÚ(	ha?Já=±—?TEŒÿ
Ûñ?wÎh3í+¶?wŒ/­Pˆi?ï@·¼Di?‹TÂPÒ=?fʍÛ\öé?fÒ7:–ä9?•#WP§jñ?‰ž8¢¤S^?ï±b¯çR¤?_Ñ@9U?kI]»?N7ÀË+q?yÌ…7æ5?Xæ‹Ϩˆ?ïnþ0O±¢?‡¹Ã\j÷á?p ,¹O+?f'=º?‹ð]…4?…6?¾B+°?ïVáÌõLÚ?'ˆã†%29?^ñÎváç?dó¢æêó?"4©wT—©?'§o΢˜y?îFïçó³…?¡*ÌýA?unk¦ó?r™'C¶y?¨ã4=ùM? (yé†?ï _ëä?€#q"\³?ƒ	eC !?k'ªf5$?'za'íSØ?y´er[vAGN4FGL J1026.9+0608?à±iR:F@HãBEõ­—À;éuyÿ À<…/PO¤@"êvÖËÿ?úG«<#?Ƨ0›~K5?™:"£§?Ó/á»vc?ýÄL`*ã¿éøÍ ¯¢ð¿ï—eýŠÚº?èËb¿gßb¿åÉ8Þmß?
^b`ó5¿Ï¸fGÐAGNbll3FGL J1027.0+0609NVSS J102703+060934?ï$=À´æ?•åЉ,Õo?I•÷¦'?;]S	=ɖ?š«§Sº"ï?•·G.%5?ï'ZÑî1?jhÍx˜?_:%vV³?gj¯.×Ýæ?‡Â·¶í?Ž4…Sø‹Ô?îò՜Ìv]?%ÐñŠ÷^?_Ö$i2Êá?P:ÌFB¼W?Ÿ§ê#є¨?Äóžú€?Œ‡&>?‡ÒlƒgÒ?S‡€T0©?Gq²´³ïÖ?¤ÍšþΛ'?‡Ýé›?îE,Ñ*³?¤Jå6¾¥?X©P/'Ô?MW­;͞.?ªçèlqŠŠ?¤@®Í±š?î´Ì^ †?±ƒæøÁG?k	;ŒvÝ?x"Íã‰?£¤2ðZU?±7QFå|?íí֌'?›"ðßüH?e–«u²ê?aù°'Ì?¯É,ŒÙuZ?›n¤
ëïà?ì#)àÏ
D?¤"a/Ä›?d_Gý/l/?cäÚ¬ûs?¾C¶¹*À?¤Ã{RLLAGN4FGL J1026.9-1749¿ï†Œå"@@',ºs-õÀ8ýN.KmÀ;ށOøÄ@¦'¥¸‹?þ™‹Ýtk?¨ý?l®?Ÿ-ڃě%?ôÈØ앿ð@œÜ$¾¡?ïÿ"­~ÿ¿âöq ~¥¢¿Üœïd|Vh¿ÜÂܾ²W׿ߣÂèG|–¿á[íœP-?AGNbll3FGL J1026.9-17501RXS J102658.5-174905?ïö¸ÝÆ^
?BXF€¡­?!´»n)?	§Â¼é©¬?PÌ)I—É?A±V‡è-?ïá¾;íõo?oO²$"Ý?>ÊÚw‹s?IGNҔ?jhh¡"'?j}&Ã'K?ñ»Å?ƒ†ÆE±?b\tx?l»z;CÇ?ˆSý±…Ä\?€Žçglp£?ïÓ«Õ®~?Vcá*Ħ?@ÿÉ~Â?#XêVˆ‹—?t
4Œþ™a?U…UÝ\²ù?ïò?Â8'?O6`Qµè?$D`F=´?º­æ?XøRNê°?M³ª—Í\?﬐‰ÐxÔ?ÃÐûÓM?P\ç4¬?\y4\ó‡â?'Ð@§ìiß?€yŠÍÿ?ïQóµT?Š×˜‡Œï?g™yTÔêe?nÛ؏Âå÷?'ÎnMë=?‰²³˜‰©V?ï—/›gé¸?rjpPeï+?SËÙvð–?@LÌ#Ä?‡ºžn€_?qÇrrFÅAGN4FGL J1027.0-8542?Ãóû'þ'À7£é·¿ŽÀ9VFíû¾À;äé@- .Q?û£®@˃?±«bï¹`ß?´×mÌ ª@PÕ¥¹b?ë@­3J¿ÕTF=Ñò¦¿à@GD¿ÛQ'Ã'ë¿ÔÁä×Ût¿à(»àì?¿ÜœŠâAGNbll3FGL J1026.4-8542PKS 1029-85?ﶁqY´|?"ANò³éŠ?T_qÙLê?exÿXÓ?§jðW<?‰Æ{§,?ëÿ¥dqL?¹§ÓS¤˜?®ýğ(e)?²V"?Ð_?°ƒõ‹u?¨³ËÌè>?ì—9É`—×?¥-zP+¦?•¼<±··?'^ÉØ8¬?µ×"‰×Tœ?£.ô¤Ì
'?åeô¹Ù]²?¨Ii}—Ã?°_h¯³Í?ª8œUjþ?Ñ<a/Dç?¨'Ú ³®ã?ï$P… á?–Ç>…Ò?p±[SaÌ?p=¶ý'<–?—PtWƒ}?"R€\Zµ?æ/n!h&ý?ÆÖðÌA©?Äۚ'_`?Ãú [Ùß?Ã%kßÍ«?¸×êæ|ñú?ìl5nˆ?¦¹Y·Þ&‡?˜%%&˳Ø?'èét3"¾?¹U	üëê?£é؈Çw?ݪ1¿<F?´?þVÌYN?¸†ŸÁcӈ? ½_tT?Ü4&PQø?µ›I¥™	ÚAGN4FGL J1027.2+7427¿íUÖ.S9@Cšù jn3À9Pý^e%À<gŒSã@rªuÛy@;'}E¥ü?°F[®ýY?µFÏóî@g‰¿1×@.[~?ëÖz•ÈSÁ¿ÚOŒ…4î¿æ!pÞ9†´¿äñ"íjÒ¿è…?\ŒH¿ëKã-abAGNbcu3FGL J1026.5+7423GB6 J1027+7428?ïö?rG9?A8·!ã´?2Êu3Š?$¶°ßmÚr?Mœú¡d?<f+î^T?ïÛøì:?pó3¢ô~?DÖk†ç?NW‹|ñ?oö{ I?mºÓf&?¶å¸_?z՟^•?a¬xp‹w¨?aLê?"ñ´2®^?yçõäE?ïØnÄ·]-?Uf–2ï?V6]Kíä©?;vvuJD?lvÆgÐð?SÁ¶þ3>?ïë…ZP9?WÌ;92lâ?BAE`ìm?8€]½è¬?_Ô¨ˆ$Ê5?T%àžE?ïˆdï݌Ò?`@'O‰²?VJÚRG#Ä?bÂi@fD©?‹hÃ#Zí?ä–_Uå‹?ïQ4W3?†=òV?l½ÀºÏ°?j€©Oóqø?'AÇíâ=š?"^tºõr?ï~;v<Œ?vðkÙ"*?sz/šš?^ûŽVŒ­?†´
¢à$?tA{WöPAGN4FGL J1027.6+6317?؂C«j@T@G}"M:"À:;ðJ€VÒÀ<¢w$ú‹L@²' V!J?þS¢úkk‰?¸ø*We?ª®NÝ]¾¢?ðïga8)<@lïåU¯µ?ïû=ù_ÒÎ?–'¿§í'¶¿ä¹xýAߞ¿Ñ>sV¿áƀ,‹#¿ëùsôÄb›AGNbll3FGL J1027.7+6316RX J1027.4+6317?ïÝø³|æþ?\²»(Üÿ?KZŸ3[Í)?@ 4®úŸQ?k0¤Çü×¢?WÀåˆdxà?ï¸Í.¥?~¯BL²ô?]&Fº?eã~Ñ×x?|OÁf@Á†?v"CÛ­Su?ïb®G?sw?|q´{±Ìø?jŸ´eͺ3?i*ø*¹\?V@ëŽÏ?xUFæfÏ^?ï\H!Ï?uå44S†r?ŽÄ;=IµÌ?m
«âu?Ž{-´rd?j@n+Qö?ïÆÙêRÕÌ?jAŽ‡A#H?Y彌€?NÛ³iÏt¼?vÊcáZß?fE°
a¿K?ï)-Ÿ¼?˜t¨Q Â?q=C¢­·?zVþˆim?–Šö¾ÄÏ?"u@0ãï?îðr€k®?‹4½T'\?tKêü…'?rþª€Ì¸
?œÞµ6ëêî?ˆ"rhFH?íšÊ%þlW?—t: ¡?£•×Pàøf?ˆïe/É?¢½†M€t+?'·xƞ&AGN4FGL J1027.6+1828?ïÿ6²LK'@Kñ«ó8qaÀ:zXËs0yÀ<u¡Å¸•@œ_.
Ú@ÕIe¤Ÿ‡?¹ÎAÒ¿ªê^ƒ"â?ð­
ê¤@є\Ãп×wCÃÏ"=¿é"iÐË¿èӓZ»7y¿Û¢ëý¿ˆì¿ããðj`Æê¿ðAGNbcu3FGL J1028.0+1829GB6 J1027+1831?ïá
Ü?dÕb¯bÍ?R£hBf.l?Q‡1	$Ó?e oÚUû?`{·»«'É?ïÎô9£9Ö?t~/eˆAñ?KO6®ØI¯?TÅþÏ«?uüN´\Ø?q tq›hœ?ïI×ëAŠ—?†›Ñ™‡Ì?v}æ•_Ë?|ö–rdJÔ?'%ˆï‹T?À7sw܇?ï°¡qe"$?b<_k?n'}ØLϓ?Uˆá¨ãvÐ?xnVȲ	?YBÃ"Tê?ïÈP?ø,?y]ž/BED?^GÜ7£Û<?Zòò|
‰?tjàæ®â?w½üvE?ïRhÖÉ?'c± ò5?dL×3Ùý?kša&øȗ?"=	Q¶¡ª?Š¹B[Ž)?îƬ ɓ?Ž;þ€©?gšï‰(?€I'mìï?Ÿe£¼ÀâŸ?‡«€sn;ç?îýk	¤L?"LH$~[ó?‹ÄÔY(ÓB?zã@å¡ý?'p2m¢à?z2MÈq[ªAGN4FGL J1027.6+8251¿äßäÆW'@@hó¡LìBÀ:Ž‡=vƒÀ<¾|ŽÆØ@^Ç»ëÓù@é']e5å?¼±]Z¤k¿ò»Úó<^?Ôå¢;~±6@-W&,¿ã{ŒhX®î¿àèh~ïtB¿äiæ÷mŠ¿æ<Ý5Мe¿áe¥«ö"p¿âÖ ž9%AGNbcu3FGL J1027.8+82532MASS J10284195+8253398?ïÓrž¶—Š?«"èÐH?1™Á@×RŽ?$—!­Õ?u-µIÜ?«'"ÿ=Ë-?ïæðC8RÇ?h¨.ù5ã?9Hý$!€*?EgNÄ?.¤?eæD%I=?dµ[ÖèG
?ï·d%"J?tâªÀ¥ý?T+HZó"Å?Vñ¿7W?CFü‰?rù"j1ýÌ?ïïŠÜ`<?=ó—ÉLhE?;˜'‹þ:'?O¯pý
?Z'ä–ß'?<ї)ÚFk?ïä›7S:?_®}é$ES?CÈfý•e?6®ô'Pµ–?frãK)?]ªÎ·"î ?ï±®±-ßâ?¢LÍE;?JÙ@¼Wù?Xª?ú?æ¿¤´—"?Ä]*f$´?ïiÃÿ"ì?…¶åû_ì?`Íý:/&5?Zå»†MC?­Àk`8^?"Øö?¦¢Û?ïÌãt`?`þC3{Ãs?TXä‹Åòn?@]Ða˜HÉ?txÛÍr?_xlçù'ÂAGN4FGL J1027.9+0252¿ïýù¶ïì@HÏÃøÀ:nӕ=êFÀ<A†l–+P@³¡ÀY¡Ý@õ±…H©½?¿ÿ²RM)Ô¿µ
…†H?ò¡öKKX?øâ£8SÙq¿ãa|¢¿ëZ¶ÐE®¿ìÐHbz¥¿¶d±Z€¿êê~äa"¿ïïK|ÖtAGNfsrqTXS 1025+031?îÌ[ã¬?½×\ƒõ©¡?ƒ¶Z î2?=ÞlcSØ?©ùŒ¼o5?½M?ïCdW²2\?šê#÷`\'?`2˜ú$ƒ?'yØ?>¯?vÐÑE*Í?‰m–ª}¡Ô?ìۀžã?¤B­Ù?'õóÝhï?2èf"?´Ü}'G²é?¢¡¯Yø®?ï25çîfP?˜§"Pv?†=W‡"	?uÐ÷•'?5.rõ?x3>!f?ìã‹\·]q?¾¯
–íá?š`KR
z2?žÉ|[?²K'ET'j?»`ãø…?íhV5kǤ?»‹¡kAŽã?™—˜â?°OBìx^˜?¬¯Z>Í·?±ÊWyÿïf?ëÖ؁kb?¦úî}‰‰$?˜|—Ú›¥?'•ªü·Xï?»*;Ó?؈?¥®të6Ï?ìì¤õÝ:?§ûˆŠÉ4K?ªhŒŠ¬/¸?¤¾V ã®?¦Í$8I¦?›ÿD_ŽAGN4FGL J1028.3+3108¿áMu@MOп "`À; ³	­'ìÀ<Â=U™@óF3@@÷U^×%ì?ÁÁŒ|Ћ¿—».>׬$?ÖÄzÃÀ‰@	¢ohî€ý?ècÆ
•ê¸¿¯Ù1½šÞF¿ç,$K8ãv¿á*`üš¿çN£Îç?È8ôhG<*AGNbllTXS 1025+313?ïøOœþÜ?BIv"Àßý?)3T	û?" °0K{?I…ü<ހÒ??ŽEÅ?ïÚ ¼Î¨?låéÍeX\??oºŸkÑû?H'¹™Á	Q?p¸ÄkÐÆ?iž‡ig4?ï­Ïcªõ7?yY´ÃÀÛd?Vb,Và`?`¾<•úT"?ÉšÒw†G?w"Ö,p?ïݜá«3Ó?N|kv¢,?NwƒɅj?2§Ö"ô?jÅ=bWt?Lu |$Ü?ïêTî!ŽÏ?cÊ tǹ?@;(.ü!Ž?;%#û-Þ?aœG¢—¡G?ahю÷(ê?ïŠÇjüçá?‰…ïÍë¡G?P¢ch?d†?Zù¯Ì?‹9ØÉQ$?ˆ'1ƒkëó?ï_¶¦ðš1?†àt.²?_<ÚžeF?^"w¹K?']ƒjz?…óõrÂÇ?7»qõ?p‡ÖTá/è?häêapzí?Rð³Öä';?‡¤whù0?oÏð/ŠØAGN4FGL J1028.4-0234¿ï‹€á@FB[åÙäÀ:",Ý®œ`À<YZ;µ¸´@œ±a;.@}G{¿"ÿ?¼9ï:
?´«§Ž#ïž?õ	Ggž@
Õd]͐—?ãi§c†¸¿åvæF–"¿è2ŒÖ<¸¿çwlþ°õ¿ìð]ºpT¿ïñÈdˆ?ÕAGNfsrq3FGL J1028.5-0235PMN J1028-0237?ï쀆qk?Ty÷)My?DR´1ñó?4LyOµ?\ÖÓZ¶R?QK×ëI»?ïÍÍc~2>?tWOè´"?Ps@–×s?Ya ‹ûž4?tü~¸s?oñÖ¶ùXs?₩6
(?oùçŽÏN"?Z`ÞOˬ&?\ƒ÷5t¼?yàu[VÔ×?k\ø±¦ÿ?ïÄ2~'g?WìàYl»ê?eúºëÖ¬º?GÙxnw'‹?rþ‰W2?Q‡3Ðcó?ïÝ"ìd?cÛÕPÔÔ?QÞ?|?B"8Ÿç*?iN\¶7ª©?`ܱH{?ïiUƟÑ?˜¾®H?`cö黣å?hqà¿Qö?Ð¶fXúm?Žpâ­4û?ïŠ\ïD`?zUbq#?bÅD»™eA?Wû*Õ¬õ`?ˆ·©PÑÅ?wt›qu?ïKÊ4RSE?xʜNG"?_ÆWnÊ?iˆSTr"c?‹­¬˜qGã?pÈYΐ	æAGN4FGL J1030.2-8403¿æÛ¿â"	À6:îA'šÈÀ:Ë£jÓ³qÀ<t±i@ k篧"@Â9櫛$?ŝ´†YöÁ?³Îð"{rg?ñBºtÛt/@Š²öâË¿ïÏAò×?ïýw$#Ë·¿ç	Ü!Ôf¿ãØҔŒê¿Þl¤Ùh¼'¿ä.1,edAGNbcu2FGL J1032.9-8401PMN J1030-8402?îÕã»J?Äuk^=ù?a"VÍÙʇ?‰ÔNþ+Ê?¡ˆŽæT‹²?ÃoO6Q©I?ïœcÈý4t?‡EØ9X	ƒ?\)˜øyš?`…+õ8"%?…aړôc÷?…Db=^p©?ï~º"—Õ}?w±¼>ùÔ²?bi(¿e&?bP#ú<¯?‹­@ØqÍv?uZæ³ðá?î‰XÎù!ê?€óHƒDÍ?€o½pgÐ?c¨>­ü±N?£NƒÐwb?€;¾Ð	q?ïoDìn'Ñ?¡[§â=À?_¾¶Á±z?uزMÛo?wÊÑÍ?h.ªœÓ?îàDrî›?™gM%©†?rî+A¤F?xÜúgÇž?Ÿ;æÈçÞù?–Vט¦×$?ï°Œ`‡;?‡}hd,1?jáqyh?e«Ñ=îwÀ?™Æ2N½Åv?†"<5Ûò?ëéõ'Y?œ¹\¨X–?"ÂO<˄Æ?'˜4ò~°?»Ä0q?œ‡j+½ªAGN4FGL J1030.4-3001?î‡w…ȁd@7¥/Ÿ¾wÀ:—F·G*À<Wé^ÓÊî@ú#d=;@ÿ\±Ö§?ljCu –
?À¸SÙpõ?õ'ÐɱZ@æ¼,k˜Õ?ïyێ0¯Ë¿è"^ß´[¿çÔ/—¿æÒ"!=¿ïÿ­_I;³?î47ûäAGNbcuPMN J1030-3004?oœ?{3‰´
'?iþÖ£•?b>"Xû*?ƒÜÓãf÷?wn)Ö¡ˆ?îü)C›5P?™ÿšØÈ~k?†4}‹&¢?ˆùÇø>Ïû?•`˜¾t¼¸?¦ 1F­?ïÎi¹‹?ˆÔÙ
È°Þ?x©m'&?ti1¾‡C?—NCqÿ(?"•M¤«G?ï" ê@%?w1BÊUPK?ƒ »SK?f‰7xɉ±?'¸Ã*Œœ?p^F®!}_?îÈØ"¸´?™ÿ–vð€?ƒ½~d­Q?~V—2Ùh‰?råï–M?—.ÉéƒìÓ?íƒÝ×Ùg²?­êÙKbq?–Ó&²M¸?š/é	•ì@?¬XÄÛ?¥''²FO?î"\k2J?•'('­?‡'"Ÿ*?ådÓ|.ô?¨8¸©
?'4)UÎc‡?íëÿ©)@?–]]ÿ¾?ž,¸´€¿r?‡Ë"*s)?¯
ãªQ%K?*žd.©AGN4FGL J1030.6-2028?ï(Èÿ@?s̪ï,À9䌎\À<.'"ø@ ]>6q?ûm±cºº|?ÀªQø›1Ê?º¸p^â¹s?þӊ¦·N@:㫶}¿å<O;§uû¿Ýg"s—§¿Ý–±Ý³$¿Ðkž3²4¿Õî¯á»v¿çø
¢gÉAGNbll3FGL J1030.4-2030NVSS J103040-203032?ïÝC]Þé–?iBš*JmÃ?E8sléÍ6?[ï½úaY†?mn…àöØ?cš"–ÿ}?ï߆ˆoН?m$_ilÌ?Cp}Ÿ"N?Jހq™á?kµÛbŸ"?h÷t¹5ü?-»á(?€×Ó¶é?Y°|þâ(?]gèj¹¼?‹æq»8¬?€971R?ï_Û©£@Ñ?m,ã>"'e?bÖ]L:Ü?Cߛ¾ö<?'Ïûúч?ku½»Ž?ïÅõëT!j?v¢1ßW?TÏojw<?Qºgê$ït?wþÖuõ%?s78¿ÑÊ?߼5?…ˆ8{Ð
¨?U{À&^?_ń!kï??‡¡P%¨´?ƒm:P—Æ?ïÇG²?tRCa6?c~7Û:2?_ëaÑkîí?œX€,‡´?ŽOâýT™?î€!¯ÁèÝ?†Ð‰5lu)?s G£?_U3²È?¥™Ü®öW?…Â0Ñ)	AGN4FGL J1031.1+7442¿äzDÃ@C™b¶®}À9×â[ªJÂÀ<7 Àiçû@ÒÛ¯"¬@j¶ÂŸLa?°/x""]¿ž¶eà¸À?ð_1£æúu@;ö%`¸¿Ú«Ä"o
¿ãóVµ{¿äÁ߇Oj¿ä¹mtw¡¿å°‡‡H^>¿'fU8Z~@AGNbll3FGL J1031.0+7440S5 1027+74?ïò"}BBg?Eš#ñ±´Â?2=ªqž™?¬awí?VIš‡d°?CŸÞ&.?ïÚî»´÷n?o²qè1Ѕ?Dðñž® x?NñÂê?oÕªS†&?iâŽÑyºÃ?ï­÷C»8?wÄ>0+ß´?T¤Âú‰q?U p˜Ûaó?í–¥'2Û?véîçàç?ïH¦'á?fђT7!?ac
Ò­?A­lò­Ø?"U<a ÿø?fºoÎ'>€?ïáÌ©™õh?_(³[û<?B·¬_'í?1»ÉÖ®Õ?i…k}g4ô?\ˆ6mòƒ?ï‡=Ñ–X?ˆÂ\·ŽE?Yåä²s?bº$ÁæÍ?Šóß=ñ/á?†"ºËŸ?ïb2ÕjU3?"à[
‡B?bgíG"0?h§ú‰ä9å?'vXRШ?ƒ¾ {s%?î²'
FJÎ?‰Å&
‰N?}ù5­)M?fhT=´^?¡hsLvþ?‰í"‰Ã-AGN4FGL J1031.3+5053¿Õßåø[µ¢@K:\|ؙÀ9$wSôsÛÀ;ñEgée@ 'äõ8?úÑW%€Ã	?¨â¢:ìª?¦ÝäIk.@Ûh‹Ú"6@{Û3íÃ=¿ëdµ÷ž1¯?±¡ÙY"0,¿Ú¬)Ür\¿ÓÂNĉ1¿ßYvɋ¿¾|^pÐAGNbll3FGL J1031.2+50531ES 1028+511?þ§?€m`³Ðx½?Sá	á#r«?D9
¨qζ?†]&/?À·"þ©?ïšSœùå#?ƒiÈToÔ[?bÝA4ã?eŽäDo¾ý?"æ!va?€Á•Ö¨X"?î×z£'?'¶§×úò?tR²€Îx?wgOùG>?Ÿüå®æ ?Å{vx?G?îU÷°r›u?ÙÇTlŸ?‡K³¾¦ó?fB‰¢3¦¶?¤Í˜½%²?~ì	Ž0?ïÞ ^Ú¬?"7ÿ±â¢?fŸ‹C;#M?^†z}֍?™°:†=æ"?'~ù†ôcZ?îëþ1?ÃT|Ô?uůÒ4"™?}ä'•œ?-Sl0!?šÙ"Â…š?íŒIg°›ò?¢P3t ¹3?'RÏÕ·c?'™žvÌÙ?±SZÆb4?¡äÁѕ5?ìl[Ç7GÑ?šSŽïÝÎ?—¢ý;A®þ?~ªKì[>/?¶´bwb9?—OxŠÂAGN4FGL J1031.6+6019¿à"ù)´@HïÝëÙÀ9qÊ0:ZoÀ;ßþiýʜ@}'î°@ח{²(?³ dd?¡A¸~ƒ‹?ìEHßlâ@/]K4²¿Ç,ý6¡þ¿åh9Úí!¿æ9ÐÁN‰¿çk%@@¿èT@ßn:¿ðAGNfsrq3FGL J1031.6+6021TXS 1028+605?ïú©I3Ù?3äA䅥?)ýöAðU?o"l|«?=¸øàç{[?/ŽPÄÞéW?ïßñBÍÛ?l"3¥­O?@\åM?I|åÑÀgØ?lãGOWP©?gíõâ}â§?ï©>¸Õý?r؈ióT?`m® ê§B?[»›Ëò¸?"æPeò?qGÕ&@?ïàˆ	¾©?Pk²€COí?GKˆejZ†?-bõ#¹¢ ?i¥1õJa?N,Ke¨8È?ïö""[?DA5kä"?7â篾×?+¨pˆK³?J"µ6ŠâÄ?@2:ÉÚF	?ï€Bt]ŽÀ?ž[
ïa4>?RöÆ\!"Q?^¥N[À3¤?Š$§A\?ý.JˆgØ?ïj$DÐ6?5à—óçÅ?læ
dH±?n	"Šl?Ž[=cCä_?}	àëÈÿx?ïŸLl52?pÞnŒ¿?düðíRL?Rá§T46?'íÁçþðÎ?mqÀŠêÂ;AGN4FGL J1031.8-2609¿è"€ˆ¯;@;ÚÂXՄÀ;bÍÞDÄUÀ<©EW"&@!"«s5Ø?ÿUdìã2?ÉRß äçv¿'õžþ'U?Ëò{Gžû@=Ü.""?ïÿå(
eC¿é#´ùàV¿å"…fîW¿ÞTÊ\°¿Ùö¢½.ʿ͘uWEMAGNbcuNVSS J103137-260715?MaL?œ_	k\Ç?K`Cdˆ?`|Œ${ï?Œe©•¼'?š'Ã(·˜Ù?ïKß¼`'?•3r
móø?p[ÐZ?t›AóŠ?'mH¯?'~¤9ŸwÄ?îxÛJ¶T?œ¸8ÍO—?]°p²Üìï?PNéÿEZï?§"ÇÐc°)?œ°T,cFˆ?îúëjéû(?€¬·¸!qÐ?aó=¬^?HUYA*}?ž€>Nºæ?€±t{ÚÆO?îÇöÒ¯»?¤…Éëxß?RÛv$sΖ?R²7é?¢÷ôå6ÿZ?¤!"~õ?îg}ÝGæ–?«;´*ýJ<?vMH¾Ð׿?'ø*õÕ5M?¦¾yù8&?©Ü«\Ó?íK5—¨?£×—°O,}?dœ¡6:v?`|ô¹ *Á?µyG´é?£ÑËòÙ½%?ìgd›`? gRWË?yɁÆÂ?mCw4P%?½x/?øWY? ËŽÞÌ?AGN4FGL J1032.6+3737¿Þ/YÁ´¸%@M‹ÐÐgŒÀ9ÞHÈÆ­ÏÀ<O[ïêß@nf'†*@°ÔcšL?·٘b7¿}ËކÒz?DzvÊ·ž½@	Â*úÕsº¿ïðÝî]@M?ïû¾½?'¿ã.$5inY¿ß:;֚׿ã/×^ G¿ÚºTDzÙ:AGNbll3FGL J1032.7+3735B3 1029+378?ïöyìQ?>	¸áî}
?.(ªÒâÄ?@ÒÏsw?NŸú†Ñ?:»kçÜã?ïÖ¢Ä:¬ú?qÒÙl€?F"Ãj²ª?Q@Âáã÷?qÞ}ÇÝ?n8¼œï^?ïÅUE?cªJѶ?Pãªɽ?C£ýO.c?z¯WÀ!?aïß-ϓ?ï»c.L	?^BZʧ/¼?gTö' Õ?K‡«·†x?v¤_É77?X²š¹V?ïð½çÎþ"?K0
Q™E?<õ°Ïç/ÿ?0Úë<Éû?WFÄ"ÄÒ?GWÃöÔ¿m?ï'xaªXÈ?Š§‹ÿåïW?T
'ƒÖ?a7%Ó¬L?ˆàBµ5'?ˆ•ø³5?ïš9ڗ:Å?uô'$a‰Š?W€,Aó²?He"K‰?†™Vè_?të]Ä>¦?ï[AA"É ?w¯~°!¬á?|
ÜoúÐ?fJQäJ&?‹(Áœj?rõ®'N-JAGN4FGL J1032.7+6624¿ìÏí
è~@F¦ˆabñgÀ:³Ò†ëAÀ<áN‡Lü@Ýòd@;bŸ1‰?Á-蛊_•?¶á@w>{?ó{X|˜Ø@&©b"?èø±Eˆ¿än"½"u˜¿Ü§A¼c¿â¿Sg†¿ä?_¼S-¿è?¸¢HiÑAGNbll3FGL J1032.5+66232MASS J10323905+6623234?ïßßéà
?a¹k8`®;?K\w´¾*?=ܧÃKlW?iHø/'¿?^Ʌ^?ïÏe…?'?rvÀ?KÉY";A?RÙëÕX?tÔçíeM?n1õ»Äiä?ï­mÏsì?oúN&ÿÑ?W·î&åK7?\ƒ6s_P?­ŽvVo¸?k¯‰§Ry¨?ff5¼Ç¾?]?؏¦	??l;:õ9Ÿ~?GeøÀæ ›?{¢G¦ÿQ
?ZÁ7(Dr?ï¼#öîù?s§ÞY¨?\6"19?Od¢°~Ž¥?zÎ7ºà?q¯"öW¾?ï_lFF­±?}P@gØ?]ÆH"ï5?dOÝF?'@ÊËjÌý?Ž9T+ó›?ï_í'úz?€;¸ˆâ-,?b´ÁÒ1î?e6ðxiÆ]?'«µR®?|±!Ér?»îG?|Ÿ¡.Ýß?äµ©G?cŠý¢í%>?"¹.Õîn?y¥‰¾7AGN4FGL J1033.1+4115?ºª™= –Û@M0){úLbÀ9ÖÃƓÎÀ<T²¡¨[Ô@¼®Ç~.@¢Ÿ§Ñ?£Û1ƒIÛ?¤ÚT¼ÅÄ?û¹St[@Úº±AV?×6
G¿àĽÛB[¿çŠèáÖIM¿â±ªÂ‹Ö8¿ëÁ+Cz©¿ïùá½õ™uAGNfsrq3FGL J1033.2+4116S4 1030+41?ïÅA«Ï"Á?¦,à©Á¿?iUß&^î?¢¿äüò]?p´:œk€Œ?'W+–ùڌ?ï²{
jð—?"K
/>)?YÍmn0÷Ò?jßÈ'‡Q?€'©gUA?{gM˜Äo?ï—Ef?"yšœãò?dm,åür§?p†Úp•''?…[OғE?'IWo¡?ïìs°Ê?Jæ1ž1??WÕîâˆå.?D4Ô0"%Ž?N…aA2¾Â?6Næ…Z‹Ã?ïÇ1A&Í?v©b:ê—?OJ-…q?@B`n¹bM?x¡Ï'8œ?uνù,t¦?ïH}›õ´?—B·ìˆ,s?g%MêFu?€fãvôÌ?"¢ûŒ
·?''8 P/'?ïH¯§fÑ?yЩå¼ê?iÏèç ?q\­6xÇÆ?"¶(ñeÞV?}œwc?ï̏ê抰?iËXÉ9Ù?pÖ=I¶Y?d0óñ‹¿?aÚNîK2?Pó0ÞbAGN4FGL J1033.5-5035?à¿Z/:D
@×ÙõÀ9¦œë]±ŒÀ;êÅ®ËZ@ Ü:Óær?ù4m)Ï?»t#ùYs?ÉŒv›gÐ@¸Íi@Yùb¼c¿èõµ>:Î2¿Ûª7áî?µÖãÑ÷,¿Ï¢ô¡¨î¿âÏW xEŒ¿âAºÃ.¾AGNbcu3FGL J1033.4-50352MASS J10333216-5035287?ë½#ý?¹ðaô´æ?¯ÿ¬	hŽ?µ1`"«õ?²èÝð"Í?§5»ßÐÇ?éGÂá*k¨?Áß`z`±?°ñ‰vŠ?'Œ'~cÁ?Éåc,Ü=?Àèèìèöú?í­Ò®­?ŸÞ.Iš<?¡­X¨¸›g?•sŒÒ|]J?­‡Ê.çÆ?–œ"¦/Ž•?ëxwßÏLÉ?™òÞ.t?×.¹%?m_܈Ó_û?À ­"Î-Ë?˜!S8–‡\?ç8¨ä¡eý?»–Ü·։?½VÚϑD®?±.þ:ðü3?Äqï±Åµ?²fs`ü˜b?âãè¤2"•?̏iXÍæA?¡6ÉY"Š«?«T÷=¹žó?ØUŒhG?˧ɼø?êIŽ"Wæ?¨^†Xpb?²#fªŒŽ¢? ˜'0?½RLàв,?¢.¸¡²òÐ?çUüÏ|ˆ?«C·ùá@?™ˆÙ‰Çà?"OØy¹~?ÏvñéØ?«1°|4.AGN4FGL J1033.5+4221?ë['T>@M{À;×`RP.ìÀ=qZ¶.ü@!gضea?ô6%UúÞX?ç`^*WÂ?ÙzH0yÿ?òµ
œ;5@Žî
å÷¿ë}Õ]¿ù«¿çÄ£2Ÿ¿ì	ۂr?ÌêžÚK:'¿Å±ÓLBβ¿î÷#"úAGNbllGB6 J1033+4222?:df?…á¥ÃS?U¾ó¯0w÷?Páûé±?…YRèÁ[;?"Óöú­6®?ïÌp'J?'Ã…ÝAg"?HÖðû÷Ðæ?_JŽ«iNÈ?v¬Ø¾°ø?2žP¡!à?î¼ðˆ°s?"BéJm?j•k‹Ž?evÄrºJ?¢‡ ÄlgC?"ÝuXËõ?ïÆÞî"ÏÕ?c*Ô(š?*D$@vè?(älð•À?{¾g©vW?cg¨>ý´?ïyb4±??'—(D%?dwâòß?m׸ïceV?Œ¢Ñï?‰ fOZÕ:?ïb´?þž?"7Ø°ò?W¬ˆ!2½à?i‹ãÀ²¡Î?'.¥xØ«i?"åpYE?íãƒV¥íÕ?ÌÏn@9&?q6WÂï?ri¦øªÞª?¯¤ƒË"«Ô?3¯'¦Ì?ïkm‰›IÈ?€èÜË Q?2…eò#ÉÙ?D°§¦^§?'H92YL*?€t1ñæAGN4FGL J1033.7+3708¿ïE]Ïõ@M¯Ž!–R½À:PêÔÑÀ<H™—ZÛ@»r‡[ÿ@bcQÞïå?®ì¿Uڗ¿±_2µ@3=¯÷¥@™£½‰ä¿Ý~7þÉõ¿éSFc'ŸÐ¿æȬŒ%=¿á¿ž{«¿Õ'‹Ã˜¾¿åTܛvékAGNbcuRX J1033.8+3708?ï!N+(š?±4gCï?k€Ý­g#G?~©wǧ?˜få?ש?®âòìÑb?ïÊ6mák&?tF7h•I?KûKæŠoy?Q³‰CÝèº?we_"EY?q B³·?ïoóÑ'$?…8í^'ï?Vޛn•?MÓ;ü{£t? À,zŽ?…TDgó`?ïg²—Ó'?p"GÛ4éG?kx {Š5?RSÿ>¸š4?P|
Opl?oàÞ·î–?î»[…Y=*?ª¡Ãø•l?sÛµ¿0TK?zª…šÌ.?¡ÎÐõ/ÕK?¨8/¹"…0?ïVJç|Gñ?®«ò'H?aÕL?w"ò?fvÁ8S2t?'ûùŒÓ l?ŒwÜ!×Õº?îÌ°~ÎX?'Nk"Žø?d"ܱðË(?`¬ÓkK]?¡òÊT¥ÞF?'Ð<é¡a?íЋCs$î?'ÿätØÃ?‹2E˜'¹?z<²)ߪ§?¬*º`0
Ü?'À¬dÔAGN4FGL J1033.9+6050¿ïÁ«ãaþg@HŽé_ªŠƒÀ7åŸËmÀ;B`	UX@?6̛@ÚÝ0È?›'Z¦®?¸ÈºI½c@ g»/ìVÖ@æ­Øë¿¿Ñâb
a-¿Û'Ã'ë¿âøÎ}¦ôÌ¿ã[+硺¿æ~±='ˆ¿ë‹µ±÷	AGNFSRQ3FGL J1033.8+6051S4 1030+61?ïÁèUœó?­í[?WZØ]|?\…Y¶¼}?y55: A§?}™Qu텾?ï¢ÏRI_?‰>>ÃÎæ?`Û •ÖO?eȕóHh?ƒYrfzŒ?‡~,`'?ï:YKð?"™°ÕEMY?Š¬èþGj?¹Æ¾Hƒ/?†Ë@¹6J?†²¢‹"?š,»?uDM($%í?e6#¡ôrµ?Vý iÿ?‰HŸf`}?q¼ÝÜ™k?ïÆI!Ô]‡?tjT?Æâ!?Tu¡ÿ,
*?Q—Ó¤·ïÃ?w¾'Èi2?r'Û­Ã?îæ¹uµ—Z?ŸšG»ì¯à?sÈPC ¨?'Níäu'!?ž6½! E¢?œÙ[5ζ?ï#ˆoÙ4?"ƒÛ'¢P?ŠæŽ>ò"?[XmÔÖ?ŒSšÈZÝ?‹Wöªúf¤?îœ%ƒ®\?'"zWù›?~z&mm7Ü?p:^@	S?¢nbó»@?Ó>zðÌAGN4FGL J1034.0-2547¿ã[­j(_<@;—s}¦À:å
55lÀ<[€¼S@P³`•'@úњ'ç?Ð?Ÿ}3\y?º4v͒?íA".ÎI¥@¡6Æ愿ìo—!Å!³?ïü4Ï¥©¿èÞ¿¾qjQ¿Õià»[¿ïÿÙiÍy¿ïù¯æ9AGNbcuPMN J1033-2544?ï'ÂGì0s?¯þ+®Hl?d‹Òÿ'W?*œ-?È?†,yLögv?¨;˜{o3«?ïÖñ†ô%?sµÄµãz?N›IåLþµ?YƒÿŠ)†,?p³Ó'ï(?m½XgTŠâ?ïÃˋ?'ÈNÉøÃ1?p*´Õy_Ž?tÛ)6#5a?™œÙ\Uªý?'1"8¥?ï‹[›\<l?gä†P"-?pDi7»Pù?T|´âB{?…䀸›?c¦X''è?ïkQêzÕ?†ÿ+½Ê°¦?l6ºÑ–×?g=HMµ4<?ŽÖ£¼èf?"Ç׬ÏV?ï‡Âɪê?‰³òg9jÈ?`…ïÛR5?mXâ·¿ó?‰íÑÅ©È?…¨ò¢ÖK?î¡0DýqA?"s ®Sº?vÛìE%2›?x*':½7?£~(`,¢?"žÝ»R>?îör'»õ?ƒ"dˆ}­ú?€úÌ»`8?pÙgH¼Aò?˜´T¯$ˆZ?€5 ;;lÌAGN4FGL J1035.1-0608¿Ì'ò*Õ@º@E•BB…À;$=Ìê)À<m"[tšÝ@yb|¡ç@cÄ*fÛ×?ƟEÀ~ŠÊ¿…T<S~"j?»3
nmñË@–Ÿ«Ÿ7¿ïÿDN
ª
?ïû—P=Ê¿ê$½Nª‡þ¿ä†ñ i,¿Ûèù¾_!¿ïÿ§ëkôEAGNbcuNVSS J103503-061204?ïÀb…¨˜\?ˆ2…œJ,?[…èûr ?_J±?xí|±…?‡Ö+ù¶˜?ïÚsŸ<¤T?mëHM¢¦X?AÐ	È~"Ø?I.XâÖ?pŒ/!xo+?iõ«d†‹?ïbÌÀ°?Š~€þ1¬?uɌðK©?w>ÈÎ̒{?—¡L'47™?‡y¢¤â?ïÅx‡G©Ú?\háôÃ?VÌúþ?Bƒ6ZÜ?wº=Ï&˜?X…dðýÔ?êȶ?§GOZ?on˜‡Ðw?tnó
H¸;?†7"­%Ük?‡4ç*€Ž?ïŒNáu·x?ˆ¾Ä.?Cè?RHœ°á
?ZõÄþšÊ?Š£45®â?†ÿlÖCÎI?î\™e,)?•ô²uÜÇ?‡Köl'c?†¸ÏUBp¡?¤cldܝ?¬²Êò¨?ï_Í#ðÜ?y¯Í]Ïgª?oڊW‹Çê?b[øÞRx?#5
å"?uᆰòEiAGN4FGL J1035.3-2050?߁àa©@?ÎA=·ñsÀ:Õ%¹Íì‡À<'ã'÷Ó@ø'ֈ¸@Á`Dä5Ÿ?ƌÇÀ'?¤>"cì'u?ß±cÚðÑå@ ª'¹V¿Ñí¼Øc¿êo4 ñ|¯¿àµ[–ÿ‹¿àæ €~®¿ègMoœ¿ïúÒ~½uAAGNbcu2MASS J10351532-2050261?ïÔâ¤
Çë?kÖ5DÈz?HޘQyÝØ?=§ùl='?rrÚøe€-?j&ŸEöõ?ïڂíې4?k=CŽ¿ZÒ?BhFzP­?J3OhÜp?pq€='~?fì#Êu‡©?ïœk-þôp?v뀳ðæ
?WŒïª+éç?^À`1ïù?…ó–ŽmÇ?u"üôÁÓ?ï«Ý[I?_s>ƒKãÿ?Z\õt™Ù}?:"	Û«??½
\ÜA7?^/$ð¢,?=ŒA[?À_s[?_;¢Òí?U;T|Ž?Šö©,C0Ö?€¡Éàԁ¥?«|½b?…˜:>­IV?SFŽ	%?]=./ýl|?ˆ­LÉXå?"tøë…À?ï6ÓG Œ#?‡‹ðŽè?a8øÓ¾"?a~{fí?–þxò¸'?†­Çã~Ì?ï­…Îzf?{yEE?^j?pœ¨÷îT?V*>IY?™ˆ¨#­Ö©?zÕuôÁAGN4FGL J1035.3+5541¿ïɢМ\@J4…]¢r†À:ÁœiW²nÀ<¤tæY@@ß-Ím²@-î4üa?Àqç£è§õ¿dÄòÅZ?¦ŠøŸ—3?ö±
Ô~ó?îM¹kzw¿æä£î‡1¸¿è,ðùÒ¿¿á€ðя¿ïÿ³^¼£à?ïò˜Ù€9vAGNbcu3FGL J1035.2+5545GB6 J1035+5542?ïå¸¬?¬äFZë#ž?çef£ƒk?¬Ýµ¦‹1±?{>XÒheð?{C4OÃWÈ?¬Þè%?¨ç(´"]­?¯¬ÁĤî?˜ÂB1Fâ?Ÿ¤$y?£&Ú¾µ¯e?î?êÖ?™µœ:¥ñ«?D÷Ž"íb?ŒM¤ ¤?£ë£{ÀvÅ?•"´š\Q?ï
B:?â|kqLM?q³£:j%?{í<:º,?‹¸ÐâPz?oÅ;E"Ìc?ï|úsña?Š–i"(Tû?~ïåŸ7X~?€rœ¯j'£?€¨Î‡¹Ož?K "$?ì ]Nuêú?»Ç‡Ë]Xm? ýÍZB?
?¨BÐÕý÷?¶~.ß/ˆ«?¶yjh'?íEŒwOËM? ¯*!'C?–çÁ
oò6?'¸÷lƒlú?°¬-Û
?œn‹dú¥?ì}âÃ{?¢¤`ò5?°eHù	? "åÒ?¨,7E°q?õfÁ¡hAGN4FGL J1035.6+4409¿äf=\èõ@Lö¸–ž=À:ó­FÈBÀ<É	<¿¤@¾_°i¿·@1"œâú6?Á¾'cò¿eBØYØ?p?¡WÝ´>6?ø¥b¥?î©?~ðöοׅ–AöD•¿è¹ƒäün{¿äùAj-›D¿Ù°}ãۇ¿í€·_þsAGNbll7C 1032+4424?ï}FX:9ô?ŒS;!¥R?[<H"É7?wsÝ–x?Fàæ¿z?‰žêÅÆ?ïm%%'j?'ú¾mPŸÜ?i•]
€?o×PåÇÙÂ?ŽQ_WÏ*è?áÔ…1ø?îࢮ¯ð?UÌKƒÈ2?…ܨ‹D¯A?…þÝ#ÏÃ?˜ýUçÏBÚ?…'é d†_?ïZëEUA?qž!°€C8?€OvÖ?f;0¢öÒ?ˆöˆ«'?g£Ç+ã\«?ï0ä¹ÓuÞ?•Án†Ç?a‡¹‰¯Yà?YB¥ì4-q?—²qŒI?"²î䫏?Íèšw? Ã¨_$ë¬?zhW'@B?"%—•¦þ?¢zH1ÒGü?›Æ.h×U?ííFÞqöú?¿¢X4='?•Fg¸«)?"<uÒÇ?¦ˆ^‡žØ?">­¤$þ?íý&rõ.Ú?‡k•?š$9_$?†³tƒ÷‰?£|%s	À?ƒ¦CiÂ×xAGN4FGL J1036.2+2202?Ö4Dþë5¡@Mw™ÅXdÀ9ãíät‰?À<oîŒ:5†@Níd	K@¾€£ÿN)?³çØýî¾ö?©ëÿ~6"?ðüÛñ¨N@J‰)4?ɶ˜ØÔ¿çL?ÿIvÁ¿ç¯9>/H¿å'^!†ú¿ïÿ΢	?ïú²œ™AGNfsrqOL 256?ï÷ÞÄyŸ²?=ï$TÝ?:v27Ïz?..ûO"Ñ?CIՋoÁ]?5•î¶o?ïÞñJt\?m…Á¡{µ`?@|œÛÝÔº?K±¶Î¸$>?mÚçEŠªê?iNd O­?ï¯V
èU-?u˜)nƬ¬?fÙ³á&ŸŸ?p"Lê50Ã?|è ¥í~?l£;+–±?ïùWoRž3?2zIT3?4"]>P?#0pU"ˆp?@`üàž?)&Õ}úü?ïóHô)vá?M'™ËC?FñÊ®ÂÊZ??'m-~VS?KêdvšæŸ?C5%Þ4&?ïŠÅ°Äè?‰j¸'(hô?U†Œš?b|',?ŠÀMk h?‡Á¦+Œñw?ïf¿k œ?ƒ°¿5ÎÜ?rå<{J"õ?vÝ%§Ç?ñô¡?}ð(ñ·¥
?ïê—×¼Y?TVÀ'a;¯?R'ŠòŸÍ?Dh=#5ûX?Y¿E×xíë?Kõƒu­ÃZAGN4FGL J1036.5+1231?™£glî@KŸ8ÅCkÀ;M♽«ÈÀ<È°­²UR@ ¯pÆf¬?ù ÛýÂ8?ßËlåÜhK?Ø6Ξ31[?üäª9$
ü?ôýìðƒ¶?èy¯†ßƒ¿Þ·";8?¿â¼g#û‡Ë¿ÁJùùUÁӿ煿ý±q'¿ï÷²ß:ãAGNbllTXS 1034+128?ïZmÂ?‹Fæڟ?fêŸ5"Û?c<	¾î.q?'ÕñÆJ_?ˆ¹<ëüd€?î˜ùú5n?¡–ÕŸ"Rb?Ž1~ó¾
?'MÊ!òz#?Ø'óÛ;?–Œ¾©H?îo–ñs 6?–o­é°þÓ?ƒˆ÷^;Œ­?'ø'©'?¤$Sw?"æáóeî?ìëáåä?•%v×Ù¸q?¡ˆýX—b?Ž%€cò?·#9ò¾Cµ?TŽ…eñQ?ï
d†ß¥?'½VÉKŸ!?s'@¿w̃?q9uãÆ?™nÞíÒ$&?'5Оóò?ìˆy»Tø?²¢íŽåëÀ?¡4DÒ®=_?£Þº1ªø?³"Ø`F?©ñsl«œH?í"VڊÙ?Ÿva›®?‡¶WDÆ?ƒ§_<"ó?°n†@Ån¿?œúRìáë?è4MhNÚ?¬¨Wp«ï?¤ çe±3	?¡±ª	%?ʐ…ý8-?§eì"È''AGN4FGL J1036.6-3741?áFÁ!»@1äëÝ3L^À:ËƳ®ÖÀ<l$Ý/ @×è
Qé@½Ðæ7?у,$¡?Þ|7ž|ØC@Ó>ÿP3@§çC?¿©¶²"!7]¿Öš$‡¿ê¿>™Ä¿ì[1^Ƕ¿ïå¹,Ü×Ý¿äU?ÓªAGNfsrq3FGL J1037.4-3742PKS 1034-374?ïŒ%tS?'ݱ…Kim?qΙöt²£?j%Y	H¹?"lXê?}/;CX]z?íàTmÜÛ?§¯tLXM? ˆ¶|¼/?Ÿj/Tɉ`?¡ï5_5Ú'?™UÌ%¸g?îŠÏæ¡xû?•ê{ªŠj?‰F¬ÿÖN&?ƒ"†Ð§Âc?¡VX†'Æ?'BèÊÀi?î)ª¬ê?'/lKÂ?žÆûÈ'?v­g¤ }›?œJõ"—?xÉH¿Ôš5?î÷df°P?"( Ê>ÁÌ?'®­/¬³?zëO¶Jü?—¼«{Q,?'p`>{~?ê-.IÇý¹?¿]J]ò#ž?·?QžŠ'?¶W"BÞ"?·W<È*?±>ÊSìS_?íMUC?¡¸î¡óU.?–m†"yâ?‹|šŠyMñ?°»ÆhzU?æâ*_­˜?êVFk\?Ÿ­rŒ8†?¶•˜evƒ=?–³®%"Oˆ?¶¸4@ºµg?–k†Ë["™AGN4FGL J1037.0-1954?æ;É]	N@@g¿rq6¤À;‡p'°H2À<¶žõ#-,@ '÷øt›]@hwhiÏ?ÊØï…忘~º£³¦?ÑM>!MØ{?ù£²½'È?éµ8%á;¿Ø×Bœ‡µ–¿éÞ@\ça¤¿Æ·¿^û
'¿é [À7?Ý¥ãߍï—AGNbcu1RXS J103657.5-195432?ïaâ¾P³!?Ž&úFW¨?[Üt]@&?U‹å¾|Ò?'àøOrß?ŒË·Úêu>?ï\Ùp…_a?'Òsö^ü?q"•Ü¾6þ?uàÕHîo®?ÿØûŸÂ)?‹V#¯#òã?ï!–Ûö?‰tm,§Û?tqˆG¨†?vÔ}§ìߺ?–ÚÐÈ9R"?…?wïb¿a?îô?¶÷?G¦•8u?y+t
íÎ?aՐo–<J?›-H©
Q?|s¯Sí?>cµT?›–]'š­?k-óL¶Ñ?bUùÂàK?¢¢?چTá?šŸúlÿBý?îQßø<?§ì¼ŸMÑ?…·ÚDK?"]¨ÑŸ?¥'I÷¦Ý?¡ÖÇçÿì?îJÂ1¤y?—Ïâá.?}èY‹ýô?|?%eÝWô?§–Úv©`©?•"•Vq"Z?ì[À(,L˜?ž¨0n?"´L¼~ó?ƒ'ÏgßÊÅ?¸4ù+ˆ?œîçF#9'AGN4FGL J1037.4-2933?æHK¡û#3@8ß ù	kºÀ9º°"rÐÀ<MÝÙe@B†øXñ@0X<×÷£?¶4J4'æ?¤$§Õ?ì4"'òÜ+@äÁp‹?î<S£C^¿åiŸš´¿æ<m8è~Ú¿à»JùùU¿èŸó»NH¿êþøcSŒoAGNfsrq3FGL J1037.0-2934PKS 1034-293?ïíñ±Cëx?Y"—!lÓ½??
8Êk-~?8¶ª'8?\Z££??TöшìHÎ?ïåhe?kÊüHÖž?<dÂêâÒN?JðÀ¨b"£?g
ؼ;Ow?f¶N.i?ï½vóHÙÛ?pǁ=h%?VËݪ
ÜÂ?UsŽs?{'Žß1£n?m1¸üä¬7?ïÔ‹jNJ?QÐ$!rÃx?WW"2'¼?7Ô¨§·?p ÙWŠVŒ?Nîöä'úI?ïã}¬PÒ?[0_
Ào?LN—"ªÿ??FÀ&Ó?en­rj†×?W:ÍmEýŠ?ï°mÌóIt?ƒ
À*z™y?R¼¸³]a?_Fœwý¸?Õ™L?€uXÀ@æ?2‰âd?wA"þ®¦"?bèô?Z´]œÀ£õ?‡ppŽ/¢?u%Ààj?ï".e™?poY"oÝä?r8Ìk#H?X—™"‹îs?…ìJ7þìQ?já'û¡"¼AGN4FGL J1037.7-2822?ï¢ì¿äå@9äÚ<!~À8½ÔZ_ÇçÀ;°uÝÒ®Ž@4Ӕè@;7ÿJÎZ?¤[ã>?¸5™ióä"@oÄÖ^F@´·Ã{?¿ß3"À¼ž+¿á‹k~(Nÿ¿æn,Ε#é¿æ³¢.hž¿êx±ŒÕeù¿àšŠ?‰'ËAGNfsrq3FGL J1037.5-2821PKS B1035-281?ïï‰;}…?R
ÙÖYÖ?F`vY_Ú?;iÞõ?V¾ßP&?LÞ^ÎòV?ïÝ̾¬p?mѹ}[Å?Fž ‹xeì?R/n~]?l‹™Y`w?hiì-ìF˜?ïˆ?¾©@?…¹áá҅ƒ?nkã÷ã?vª²´Ú?†Y‹ñí?'À"|Ò ?ïëC·Ýõ?FñÆÔ9^?B›èWýö?+¶KÓ{?`MÎûµG?C".K	þ?ïÙíÌ:š?g8¤¬g;?Qg«8)€?F½nl™j?n4<jbù
?d¬ºÉ˜!Ž?Z1N×?…÷$TO?Z;ÅUm›h?i|Ç%–Ü?"V0Ã6»?ƒÉÿ@$!?ïÂä8Æ?"ôعÒå?{¾¨'ø;?€Õ¹˜ëõ?•÷ùR:*5?'¥'
t?ïÃG¸–#?g}ELC?]FNl—Qo?K;‡'·‹?w
«Î*+?cÚ`16ºlAGN4FGL J1037.7+5711?ᨣÐk@Iäh3Æ*À8óz¶ƒÀ;s¦#×þ@ψ¾Õé?ü 
¡©2"?›
ß"(¹?²n+Â%©Þ@MÙ<FØ,@ rIs'r?îø^ õ-"¿ÓÕ-¤(ï¿Üw®F¥¿ÙpÜÁ·oî¿Ý{C&E¿å½•!dԖAGNbll3FGL J1037.5+5711GB6 J1037+5711?ïì•b…äº?ZÏ/<Syl??1è =??3"‹^Ù?_ÀÏ+·j?Yz§~p1?糧|~'è?Ýß¼ºE?]ži0O?aûféÈú?'Ý_Ût'É?€W"ÖÂ?ï©îàh?"²àdµ'?g1F½1?w£©Zƒ?pmTÜñ?'Øá'T²?ïs"Ÿ¯ˆ?qÛàÎzä…?j¨núVÄB?Qÿx C0?Œ¿iüŒÈ?pÒ	ýü?ïì¾:ƒ(?Xs«¤+>'?4Sœµ	ÃÊ?)–êÈÏ?`·Rg'ýj?WM¸»ŒúJ?îü¾^
ì?¢.·oå¸x?tMßg³?Œ°´PDµ?›T¼v¼•Š?ŸlÝS Ç?ï¬_êvUó?"6ŒÒ'±?aY×Ü#B¬?qá±0Ž?€'o)D¦?ÌŽΛÞ?îâ.ݪ?ˆõýÃpÊÇ?x!€ŽFÞm?f´û—¹P?±Ý9)âê?ˆ<–ÔÛIAGN4FGL J1038.2-2425¿âô!Š"C@=BDËáëÀ:Ž¼ôµ4À<dêúµ=d@^ou®­Ó@E$Ý/?¿á•¦'`¿žó/{Ý_Ü?ÞbyœÏ3@4J5Ù*Ô¿ÏΧBy¢-¿ç nºu\¿âŒŒÀÃ)5¿ã ¸§{Úl¿åšŸ˜·¿ïûxçrjAGNbcu3FGL J1038.0-2425NVSS J103824-242355?ïõ&°÷aÔ?E¥pkÂ?4®2›‹?$+ŒcÁ!?P‡ÿÑaÕ?CÍm0X?ïäÈG""Ã?lª×ìÿß×?<Êûô¨?H«^º—R?gžX½}ÆÍ?h`.hœT?ïÃ<áehÃ?dՉ3@ÜV?RÕgŠ"§?TöÃÕ{Ó?y¬5ˆ7ˆ?a…¹nÊXÁ?ïÚøFx4o?Mw*芋?AžbÚmË)?#D§Ô{u?pP`5Ïå?LPmmŠ¼S?ï蕑]q1?[<xãŠä(?FHLjÈ[?7FðyhB?aâÜ.m¿_?XgB]3i?ï±hU(üN?'àŠüi8Ñ?IðÎÍ%Dg?X䌬Ø-?'ÝÌÕé?¾§^íåæ?ïŽÌ¥›Â?zåa4¡û?^|PÉËZ?Z‡é˺˜ã?ˆ©BÓ/?y=Üß0}ÿ?ï"Y"4Å?pÔÍñ"Â?YCøpÄ­?DÖE´Ñ–©?ˆÇ+Zô.?n»pÂËAGN4FGL J1038.5+3926¿ÔPœ mÄæ@Më¦ZÀ;Â:£À<éD=F²l@%¹r@¯;Ý%àd?͎àÃy¼Ú?²–ŸOwH?æ(ä$Ø&@Q-mÌaB?ïý÷Cõ"?ëg™6Jÿ¿æ9¸RÂD´¿áuú"pmP¿ïÿõEq#?ïÿ""ÆAGNbllNVSS J103845+392736?ï ¢j0Ë? ºý®¡PŽ?'öôø<Î? ÂU`ÀÆ??fݹ¢¯2)?]™UÄ0/Ã?ï¼Ë'»!?Yæ"Ò>?SH	òVú?cƒË €ª<?|È4Ae"?x^"Ñå[&?îb+A³dØ?œu‰Šµ?†üKëeê?Š\8_³?¤8ìƒì÷?˜!µì½VX?ïÀ[ò	~?bš@27ô?dQÔËT?Þ?Nƒ9^Z#C?u©©Žñ(?^Ä¡œ%DZ?ï°5¯å5y?"yG†%ÅI?pˆâ?
d?'0Ä/z°
?w\Eå¸71?q	¶?ï\Ÿ°?'|£Lr_É?aw€!õßp?jKúîµã!?'=/žCƀ?)á(cd?íG1('?¢6½°Ë?Š¤ìkË?‹n:Ô?°=	'1we? ƒ•_óç‹?ï2äÍä=Æ?'ä:	5½¸?zÝÑü:d\?n>¡¶&¢Á?'ëñ¾g#?hS‡™kAGN4FGL J1038.8-5312?áOha×û@ž!S6Þ¹À8à@
²
ªÀ;<ý7Σg@j ñ@¿,0	³?³Åé?ˆâ?ÂMŒ¥ÀC}@¾ó
N7›@VÌ=…Ç€¿ÙXVñ?¿Üôï#¿èçóߋ@e¿ëfL€S¿ïý—¥£"¿à&OÀ1³×AGNfsrq3FGL J1038.9-5311MRC 1036-529?ïژ`ù-î?e¹å=(Ï?F
@îì¥?>*ÆåU4?oäûãªÐŸ?c‰$H`T?;ÝÚ?—UWiV,s?@rx\µ'©?Vn"¼üˆ?ŠIPæSYå?–Äqúè?Ï?îG®ñpè?™ÏN»h±?ˆ³¼ãÿ!?ˆm#]Áëâ?¥"±Óg¿¯?–äè‹T?ïíáD³±?HXMÁ8?!Z­*""?Ö'ZyLŽ?a	F¯¢©'?G+lêâÖ?ïWúª?~˜h`vkL?WðýÁ$å ?Uvċjk×?…¬CœhÕ?|kÀY¥'?îê†öÌ?¨‹Ô3CZe?Z¥Å'(?wêwcTY? 'be7Ø®?¨Ë,.tA?í[À	×?¡Œ)çõ?•®Á[|?ðò¾Elé?¯{¨aÆ_?žÛÓ¥ÙîÉ?ïÐ9'E×?h''~Ü?92yµZK?-Æi
A?vP¸ˆàÍ?glVàZÊAGN4FGL J1039.2-2848?çУý(gÜ@9¹:'£À:Ý¢'vgÀ<5ZŠ[@ G5««@XE ›€ú?ǘÓv	F¦¿ƒXÄx{£?¹'FÀÙ¤w?åЏ"Ýó¿å›°å"?ïUG$¿ˆ¿çРa3÷~¿ãÃ?ñBοÝJSá)¿ËòEžÅ¨AGNbcuNVSS J103921-285009?ï02´‡?£Sô#÷؞?^Ç!/,?Ý?aŒš£Fûï?˜§"¦b!?¢ÿ0ûŠ_?îüÿò‹?¤ºË·[É?‡å7d¶²?'³Åðͳ?›¬Œ´…†?°ëj¨²•?îhÑ1­Äk?—œi%àÂ?"À"ö•Ê·?†ù'cÖz\?¤BÇ£2ã?"0âñ³SW?êƨ‹z?›y'
~ü?¢•"ƼX?ŠP‡¼SV4?ÀEzf+5Á?˜"¬Ñ¡÷?îQ0	Ýú?¥9=Æ+•R?pjr ñ¦?nHÀ#ù.Ø?¨áþ·PoÌ?¤`æýš?ìaøÐg.?¸æÕr?¢öÀ,©¡è?®œÈ°Û?³tÛìßÞ?°	V~²z¡?ìÖÓZtYˆ?£Rc~0W?"zÆ1â'?'…Ñê¶Å?´*³ R†»? dÄs¡"?ä
U܉?®ˆ¼&·Ná?²Vta€í^?¢Áš´^²a?Ó<H;";ó?­¼¼gŸpAGN4FGL J1039.6+0535¿ìÀ²ß±@Iüj%™íÀ;(D9P"À<‹RË~îó@!È¿¡ëù?ÿ(¥ߙX?Ä‹ªà¿¿¬ÄŒü*S?élIŸ†B¥?ùð3§!lŒ¿êF~3⅜¿êIEßaô¿åÎ	Bžá¿ØYɟñ¢o¿ÚKXC
ñ¿À|•|ÔfõAGNbcuNVSS J103940+053608?ï"ö׸8@?;º&""î?LðO
QŽ?RG±laŽ¤?ˆóEX½á?Žkƒ/­œ?ï))>½ªñ?œÐ2ç*i?{ß ä=?‰ðÒáDñ$?"`gÒTÕ?"TªÓÝö?ïZ¡dqÍ*?€ËKKº‰ð?a'®wÝì4?WAò<Âà?'y}š_'7?€Sñi›Ah?í"íÓz?•ÛÚýÎ?zž@Äš?e6b¿G;?±µ2òޓÑ?–4RÒf½ð?ïFº0§?'|6š6p¬?UáVÎ]?R¹SéaÖ?•ÊŸ"14P?'½Íãož?íÞ>Xo°?²s͕ë&d?†7É¡{?'Ó:ŽÂ=?¬›L²l@ž?°«MßÙ?î»Éÿk?ö¾6&Æ?iGÐáEàù?d²!UJ_?¢®é´ ?Žö-ùugÚ?çzêR!hŽ?±¿Wò+íI?•=G°¯?‹Vÿ‹Óí¯?ÏrOTf?²|°á¦üîAGN4FGL J1039.9+7326¿íK…æoœV@DF~RvŠÀ:ÕüÍE˜'À<Œ>õßÎ@€®É"¾@µý}nÁ?ÄHGAˆ
¦?¦ý&Ô!¢?Ǥõ'Î{ù@W¹‹Ò[­?ïÿý²Gæ¿è7Æ´{G¿ç7"DZ£¿âÿ¤àõx¾¿ÝÀ‡å</[¿ç<V]çAGNbcu3FGL J1039.5+7324GB6 J1039+7326?ï֍Š¡?dM´|úÆ?;VK'ÁQì?-
þÊF$?s®›?c<'YE?ïÈF9d•?pÝì±V=?IsÅPû?N¨ WŸ?x®j‹`6?m´i‹º?0š?x^Újh?V,¹—‡?B¾+Eo$ø?‡"\´N
V?x4i6JúÛ?ïµú>Ӄ?`8©æÉ?R´j‡ˆ¢?4-ì=?ñ?€ItŠ—?_ù@\2N;?·­£3?}ÙÜôBøš?I&ùh'Õ?:ø_#̳E?‡ý⢳°?}"å'¢‰j?ïnûòîä>?ç›šý?TX¥G÷ŠA?]PÍò?Ž½?Ú÷V
?Œ@Í°dœ?ï5}:ñÌ?ˆ›¸ŸòÌ?b Äª˜0??c'Å­â
?–ü@×à"?‡ùºuð¼?îò‡µ§¨a?8¡"Ï3Â?o‰g|ûÑ
?Zørèé?½ÜU<-¿?u	n`AGN4FGL J1040.5+0617¿Ü'ÀÁÚ3@JK¼'cÀ8®ìúi¾
À;éOâ–b­@'gÍï@ߢºª‹Y?¡­&ê$¡u?–¬þG»wÝ?ò'b`Ght@ЀÁÜXÜ?ïš	`ÑÑï¿âsù+Ðhc¿åf®à¨¡Ê¿ãùÓá>ó¿ä` Áìt¿îv¼àE¥|AGNbll3FGL J1040.4+0615GB6 J1040+0617?ïó¹"uö§?Odƒ±tÖ?*Ó×Ý?Ž?©ì¬Ò¹?U3[Jt/Œ?MÙx!µ]?ïÓ4î§ÆŒ?r2Õ.‹ÿ¶?E÷¾M¡»¼?N´‰äs°?s¦ÿhiÅ?pt%ðH¾?ïŽ4(P¬?†[ØvÅ?Zº'1FÄ?c™á'ú™²?‰£–êà?…˜Ù_•,q?ïë¾c—Bì?Häz¥9;?IùÅ,ΐC?3°ã	¦3Ð?[†Uųk»?BԊüe¦?ïãu~Ãe¬?dÞ´9ÊO?9ó!¢?1'ÑÐU?ig÷Ì1?c"ÐÞL ?ïu'ï†Ó?•¹ÿ€]?X}Ù&¦Íª?ekiñv¦?‹‰'ßב?"j	–Ô-Ä?ï%Ƥ]?'Á|}•Ý?e¼á "˜u?l'v¡ ?˜[{q~?èôèÎ×?ïÌX[?fŽ|š|?b²Éº?U	X£?p¥ÊŠÁOA?_Êvˆ«áIAGN4FGL J1041.0+1342¿å¯
ß0@LcZ…‡"ÞÀ:åA—z©À<'šÎLÿ@ æã'áït?ùj;rœÕŽ?ÏSƒµ¬ ?Í2›ˆ²¼?þªYö›s?ÿT<xl·¿íO˜ß_vˆ¿ÖìaÝÀþ¿äCŒ?Å(ggÃ2Å¿çDÊ•Œo¿Ûdçî'CAGNbll3FGL J1040.8+13421RXS J104057.7+134216?ïʯ§*¯_?iZ¡'³‹?QXx<~ÂÈ??ËF2›½Ñ?vRh—#ä?gv(š5ÈO?ïƒö%OŠ?‡)Áäòù?g¶ÁÔëd?k 6æúÖ
?‰LÑóZÞ¦?'òç—j¨?ïR»À¤º#?·øºqlˆ?mWó¥2bÖ?b¼Â{(­?'ý‰|AÏ@?€Oð§I9î?íóÛàÍ
?ˆáνüf?‰Ÿiô,¼?r°«/Îa¾?ª}Z±D	?†i|u]­?ï¡ù'Úˤ?voÞ£N¥0?]­%
P?MfŽÃ­ÒÅ?ƒÌXõg?t•
IÍ,?îB5ë°y?¦ÀƒÂ†'™?ƒ6­-Š?•Vù…Z
?£1b[fn? ÇäéJÈ*?îÅT×s?Œ'?ê8³õ?y_3¼¤òL?s'ìˆB? 'إݚ†?‰Þã¼Â[?ê¾Wº\?¤²ÖÈÍY}?›;5(?Ž"ÓUH²?ÁŸ>¶Áj?¢÷Û3æäAGN4FGL J1041.1-1201¿á¯ºö>>@CÖî<³åÀ:Û·ìj÷ÆÀ<'á>sÙ@l^iAâù@‹QzF<?•5[×l8¿•õ¦4݂R?ӔÍí^<Ì@}禺¿?ïþòNf•`¿æ°ï@ëÁ¿ãøɪÙ\þ¿ÞBÀÄÖ´¿å/{]™c>¿ÄZÍÖâû7AGNbcu3FGL J1040.9-1205NVSS J104108-120332?ïÄjïüÁv?h­'mô?EäËÐø•Á?3¸þËìä?{
î 2ú?gÄnØóp(?ï«Ïٓüï?z<ñKQû?U'îŸù?Xò]
úÏ÷?'[«×œ¥?vi`·gð0?ïr¦`ÚéÏ?uó^ú¾Ïí?aD†d¨Š?L{ÌÛWЪ?b·ÒŒ!?tŠwöXLÍ?ïƹ"½â?drÇËį?ef贍O"?CHP)¶]â?Š´—{üŸ?cՓo.ô!?NùŸ?wpwë?R|¼ö\)?B‰ÜÀ1—v?‡Ì"­F€µ?vÃ:š¸*?ï;Ïÿ²'Z?'!iöØ}Ê?^Ìð\¯p?b_ÔJsW?–™1]"½?' £$â?îí/Mq?ˆ"¥¡ƒ«˜?mNh-éÚ¾?^ðµ!XŽ?ž°IP¯Yš?†¢¥™½u?îc[巇õ?ƒaø¤á0?€QÌ.võÓ?e;Jé'3Y?¥µÎKCº?'o"ÿÏõžAGN4FGL J1041.3-6437?ë²£1ʏÀ¸"~–À:FU-XÿÀ;É'§
öc@æE'ƒ@U0 Y;Û?̉WW)Ýt?Í(˜zŠ¶@.QYŽç@Gì.'ãÃ?álÝÿ$7î¿ëz¥î;²^¿ÜN?=­Š'¿è©]&KÄ$¿èŒM€¼S¿ïÿøsCÄ{AGNbcuAT20G J104117-643103?íz•DAÅÀ?ª˜,!Àí?}҈gý‹?‡~g¹ø‰¿?²N-Ycé?©†'BÔ(?è(]<y¶ƒ?»iQ–²M?xøÝ©a=?{zä…w¹û?Î–Ä ÅŒ+?ºó´îܝ?ìQÈf$ó?£¨@q!dÛ?‹lÀÊ?g?'·Þ )@Ä?ºÏ8
û?¢ÅÒçÖÙå?ìϙš48?Œ½¢º	
¶?'£6m?aŽd—V?·AžÉÃÓ¶?‹ânU»KÛ?é‹pT.‰?¾Y/Aó%¸?Œà§¿å?ƒö$7Ùge?È45Dc?½ä¯pà+¾?ßwÌ&¬©?Ç(ÁôVª?"'·ñA¢í?ÿCò'?ßä'ð?Çöà]ù?ç®Çw"v?²y"ÌûÊ?›(k
}µ?ùGîÅß·?Í⏁½¯Î?±ª(Q}­?ç«Çþu«?¤¸YÈ$DÎ?"bo@<¡•?~Ț#hÉ?ÎĒX¹2?¤Ÿâ»¤ðáMIXED4FGL J1041.7+3902?œOrj;ï@NEž:WëÀ;&¹f¾zúÀ<í¬v0@ –$d
q?úµE\*£B?ÌEB;å?ÌHäu_þm@ˆô'@–Ó–•ƒ?í0G@0q¸¿á<Ybþä¿Üï|ÚÇm¿ÁvÀ{°¥¿åÎUÎh®?¿Ö² c¢¼®AGNbll3FGL J1041.8+3901B3 1038+392?ïߌ	ß}?[ó8ܔe?Eðdñ5%À?4~Èâê¯F?j÷ßÖ–?X¢€Þå» ?︃"Œ©
?v¤\î,?R>îȋ"?T6BÚ_¥_?fÇŒ?t~]ù¼a?ïˆZ–ñÀï?qÕÕò˜í?cwÿ}ꊥ?\AԛÙ&?‰Z^í·ƒ?m£]T|S˜?ï8ØØ/Í?qGsÓª–%?u†¢¼Cå?Xé»5þn?"ƒ<D…¿=?o9̒ZÚ?ïćb¸y?j3à8UW?QM½"ѧ¥?A–NT–%Ê?yhߔ/	s?hp¶S,?ïB"	œ{?'P	ÊÝ?d±â€ˆ9—?n2c>¡à?•B‹Ãs?'$—|"?ïA·Ž…?ƒ[¹ögm?o"˜¥å˜?iŠJ>c"D?˜3äȑà°?ÝŠ6³›ý?í´hŸÑ—?Ž–d¾˜?‹ђ0#?wlëâxòæ?­ô~Ÿ{?Œl¨é¦tAGN4FGL J1041.9-0557¿ïTSaÚn)@F95" ¼8À:}ïunA&À<tރ®uÊ@ C?F'ß¼@y—=žÇ?µ]ÉòíÉ¿°Þ-mÉÝ?üTDZ±?ýƼT¯"½?ïþþ๿èL[B›Ûé¿ãÑ/"‡•¿àqýƔϿÜiµ©yŒ¿½¿¨L÷?AGNbll3FGL J1042.0-0557PMN J1042-0558?ïGà³xVÃ?'‹­Fyn?W°§"|U^?LÚþµxa?•ˆß$LÂO?'<€«·?ï¸ò5£6?™Wê&îº?}Èˆ'Ã?…™—×|È
?•dï´Q'‰?'g>\ïàœ?îì×G‹@!?|ûç.Ê?p–cŠŒ·?rûš{Òðd?ž?~&=ÚÁ?Ù
š>Ò?í•Ó¿ÿ?Fŧ¸—ì?´ín>2Q?q¯^‰??®HY]ç?1¬2iù?î¨É"Åì?Ÿ`ÐbÝò?hMT}úçp?`~J0àÔ?£î™X¶¿?ž²¥FZ‰7?íjz""ë?°ŽÊE?'Ùçd*?™ôæyú x?°5±££?©ï]ßBëï?íöl@E‡?œùKFT—?zí`°?zFt¬ëª?­WR"ö?›n "6d?èVèšÔ?§!/®üÿ±?ª.ìô"V?•	Š·6_?ÉBéVÑÜ?§Æ RQ¿AGN4FGL J1042.1-4128¿ØZM˲@.Pð"aùðÀ:×Ûô‡ýÀ<u]9—@ Îvúmˆ?û38Vˆ¢Ñ?ÅÈqÞ¿"~?Ïm¿$˜'@È\$Ä?þÄ·ÕnݿՁ¤k.Í?ŽP:¿Õ¨#>ߏ¿ÀÃ*Œ›"U¿á¬!±€–¿èT5vÚQñAGNbll3FGL J1042.1-41261RXS J104204.1-412936?ï›ü»'?',ÙR?iÉñ¿55?~c¦»9«?'ŽTÒwT?s"«ïF#?îtžPÉ­D?¤%{z¶?'€à\˜ÿ?–
}«¢;Ç?ŸëUXÁñ?š ŸÀv¾}?îñï0ŸÁ?Ž'ɾ<¡?ƒÈÍnÊAd?ƒŒée1?—ݶúÄ%?‡†bÐǽ ?ëÕδa#º?=3ßwì˜?§MMêb'?ƒÇ·šy©?µªãjrd?‰5`ueѤ?ï;y¢G+ý?‰¼}§Ô"Š?zš¡ná\?q
†ãuæû?'ê#T*ë	?…NH7|C?ëÜ­õ"ŒÝ?¸7öMæ?£ÕèmPá%?§‡ÖŒ^à›?·/œ)?²f©+ðº6?íö\·ªÀw?™ø8âÿÑø?Ž=ÏႦ?ˆ
y8›¿ô?©
Àˆ§Ì?•¹
q:|i?ç)‡:œ^?£Òü+ðî?·;çö׉Ö?
ƒ«ƒ—s?ǻë?ž¢m'Ë þAGN4FGL J1042.9+0054¿îÀ+)¤i@HÄ$¢v·íÀ:½°}á­/À<qÈAíá@!º˜AÕ¸?ûÀ…`ýpÚ?ÄÍM¦&ð?­orÿ{ö›?étÀœ<â	@½±@Õ2¿ãЯgÏG¿Þå8Ô\ä¿Ý´	½#ã¿ÙyFÄܾ¿ÖÅl†;¿ÝÿePfËAGNbcuRBS 0895?ï¬ýfȋõ?uîi-Ê›?J9s ‹Q?7Ƶ>-Šç?ƒ©t?tëÉ@±ç?ï°eÿÊaI?|vƈH?S&æ¢7?W?Æ^‡–€?®{1m?yqˆ‰Iù?ïp0'î)"?{$¼³´&Ö?c)&ü®eÓ?k3d"é?)'¶Û¥¬?w«†7.n?îÎ쌰§þ?{;.épF7?ež(X¾z?KõâéÆb
?¡¿ýT«³5?{Np@þω?ïE†%.ÉÓ?‹å­Ø¼?\«œçYþh?P¯¹_ÛÂ?•""ð5¨?‰Ù€wí?ï$ž,GÓ÷?—Nîïo5®?b/c¾•ûH?péjY"ƒÑ?™&NòqÃ?•gCŸÖ¹O?îÊl#®t·?Ž
Â7(ï?g³Ýrû_Þ?eƒAÆý]—?¡Ýÿñ"•?Œ¡yçìp©?ìjó—•0?–t'éì?z!vâPgÛ?hj5~– Ò?»KÚ° €?–låk0AGN4FGL J1043.2+2408¿ÝD»»ÏÇ@NƒCc,CÀ9e"7ÉÀ<EÞ)ìb"@½×f"@_åÏÓ?¬6ÂZOy?ªÛ½ç'Ý?ú"Ô%†¢F@¬m™‹Ô¿Þh_ž¡¿àB1Ó·¢™¿åWøyùÁ"¿äÄÔævÁþ¿æ[¹™ê!q¿å÷]š
_AGNfsrq3FGL J1043.1+2407B2 1040+24A?ïåÓ1Ñð^?^U#¨Í?8÷ƒÈ"f+?*ía8¢9?g
ÝâŽ8?\lVòØ^?ïÍf^a?s8EY?M±kEUm?V³¥ôBÊç?u–ß*t"?o›Uë?ïdâ?g—&šø?RÞpŠÂìB?<	:Võ"?z<܎
¯Î?f9ä¨WŒ?ïÒÙlK
s?T[)hy|?b2²Xäe?DçÒ@ºêQ?jóá¦[‰?K—(êþmŽ?ï®þ˜vÙÑ?†›ò—ë!T?Kõ *Ёç?@íÌAM ?'€ÿä»!È?†<EbÕ?ïrx³šø?Žq@"ámò?_JHëW¯›?h*X¿ñß?r˜º%Ê"?ŒQ¼^‹=Æ?ïŒ;¤¾2M?|¬[¦	Ÿ?_0»¼à—Ä?O~wúKý?‰
ÿbvAÑ?{g`3î?ï'Â]ï/´?t羸³un?zÜðás?dĽ6'E`?'@úR}[?lQ½ø̗ŒAGN4FGL J1043.6+0654¿ÙZ@G¾z@JÆБ}kfÀ;CT¸¾øÏÀ<¤lõÌ @ `Áïy&@#gÁLf?ÍBœGHéÔ?}ó0e7?²9Ž‰@?ÿižª%¿¹aǛ4¤L¿äPpZÛï¿éz¿8åz¿Ì¾MØü¿åb'q	¿¼öLWFŽAGNbllNVSS J104323+065307?Õ?'ˆYtHMã?M¯Ÿþ|ª?X `ï?N±?‡Ä?'cµÊ?'Lf	¥?ï'ÙlÔzÒ?Œ=Kü6_?a××ޞêe?d£ñ|{›î?ŠÓ®Ìbá?‰p*!¡d?ïm"ÇiOi?uÎe¶Ëü?apé­¢u?WÊÅ|q£°?!dRǟ?t`˜h7?ï4ýþs
?sIµÄ³#ß?k×J¹;'?PäçÅ|nŒ?•ÿEA"ù;?rÛº¨ì8?ï€_Ê£ˆ?'A*ì4•?Q9–Ǩ°Ä?Cþ,§Oi?ÀÚ«P³ô?­'œÐP}?î²Cø¹ué?¦Ä—èø#(?lˆDØvã?vÈ
™ÊW¯?£<({"?¥ñ)X«ø?îÿE¿kª?""Í%,ø@?g²nɬœÚ?WØÛt–‡? ú3}Ôï?ƒXÀ‹uêh?í\þ˜O?'®Rhv™·?'[–µk8?pk"´‰?²ÓJÃd?'þx=âAGN4FGL J1044.6+8053¿ïîÞøüß@A`»ÛãÁÀ9hùi
	ÔÀ;¶˜–dZó@ÓÕ)½"@'pOô4?²Ìx±—'?˼¤¡4™@'ÁC+λ@Ö»$,/¿±@}sž2¿ä(>ãjž¿ê×ÑÍmÜ¿ío±"‹c¿ïý"¶
+¿ï¤ÀßXÀ‹AGNfsrq3FGL J1044.4+8058S5 1039+81?ïZßYÂ>)?'•î)Ãç¯?'z›#GÝÙ?"¯wL?iKÍ^œ0`?e±Þ,n9™?ëƒÇ
¯í?½ö»Cô‡¸?¶M(QغÂ?¶Í±÷ú/?«)>,r£?£EZÔ«?íÔxA§Œ™? 6¹Æ!òJ? ž"š@ùé?–÷"Ë3ø?¢÷Lþ
‡?—)"®Ã±Í?ën=†"z?œ¸
÷>‹?µApJCYÂ?–Y摟A?²³Ȭ›n?"îFƒÂι?î]Ïåä~?¦¯l''+›?§	X€t?¥Ágç	?y2õgùøû?x%¸??æ-ËÊe¶¶?˒ϥð%?È?½/Jñ?Ç1ƒ¡›×É?¾e"2s´q?·ŠxØ°?ë̜ß&õ?©ÎÊqákV?°škqÃ/Î?¡}H¯`4?±­")@Œ?¢#•OjÈâ?à­%Î#lŸ?±Êç>T?ґ'ð‰ëQ?²àÏÔCÁ?È)æ^vá?ª¼Þ²ÇJÔAGN4FGL J1045.3+2751¿ï²eîFo%@O
ÈuO7vÀ;<îM®ßÀ<¾TbWãí@ ÉýˆnU?ý÷¿¿ž!?ÅùcX¿ß©?o"=Äb™H?¨ÎI¾SÑþ@þߨF°"¿ïXPŽÌÝ?ïø]¿xÑM¿æ	°Š`A¿Û9ä<Õô>¿ÙiÝ^•a§¿ØÀäa>yAGNbllNVSS J104516+275136?ï₡Zƒ.?btù,ÎSƒ?3م³®Ñ¹?&ØJ´1Ɩ?k-ú·q?a€=Î$å4?ïàSUAR?n5"Ùï))?;'¢sW;?EâœN}ä×?l:gGËeV?j©™pæn?ï"EËM?zåܜ…R¬?Wb«Ÿ?EÇ?WÆÌ9gÎ?Œ
i+/<?zșþš?ï¼átñø?_ÎVúŠŽ?QØ~Wkœ?9qÂ{ŸV?}\±R'&?_0g­^?ïÎÖ@$C'?p€îhF?B—£ç"ún?7Wz›O?vAëTó²u?oWš}e¢™?ï"ç·oÿ~?‹"(Ø·Ô?P
µàŽ(?Y•üƂf?‰[[$Ñ·?Š{)yȄC?ïŸqü?†[ÁAµI?`("v›9?\¿œWúë×?šG
a´[?…Aly(tŽ?ï?\ÐC-?z'ÇÙïU?e°ï¿Ê"'?Tqw㥥?•V6mzVÞ?zù
6»#:AGN4FGL J1045.8-2928¿éKS·¦ä @9éã%Ô¦À9ù=¾§pÀ<?
›dtõ@…|Þwïü@ý.^¸<?¹ýjúIݚ?¶™_·ö|?ú¥)ð"R@uÏCtžã?J¼¼´¿æl¸ N¿è	ò&ùi
¿ã!ý•Âu¿ïÿù_|è3?à
 ÒH7AGNfsrq3FGL J1045.7-2926PKS B1043-291?ïðи¥Š?€y
•j?CЈm<??]ðxy<š¤?Tw–Çz¦?xÒÏc‰¡?ï嘺eZç?o°ÿÕPê?=-?Ðu?Lê|²×Ï?fµeŸ»ux?kß&
]?ï¨aVÝò?zþ³ä›c?lMëíb½9?vE°Z®Ü?}¨^íBŠ?pQ•²Ðët?ïõÕ?	?7ø/¸œ?0i	F,"Å?Û
AG?QÂ$èÊ1?5ÕÏIð??ïñ˜'(Ÿî?Pý¶G!ï?H¼*¤æ?BÌ~<«µÜ?PpøéõÍX?FˆÌ3¨ãf?ï¯Ñ/n=Ü?ƒ¼©pQ£Ã?Iʙ—L1l?[B Xæy.?'o
…-;£?Åqè¾XŠ?ïVó¨iý0?ˆ
o.?zë¸úJÇï?'a±Ó¦ ˆ?ŒÍ9vqµö?~v¥æ´Å?ïÙ1ø¶Õ?^ræOË\o?Nÿ.~p÷:?=²cftåu?o<%™›^?ZmuÓ¡kAGN4FGL J1045.9-2331?ߝN&v@>úÓØYÈÉÀ:ãHÇïî:À<'âÐDP'@ðëzŒãÿ?ÿ.˜I7w?ÚÏyº×?×¹ügÅ?ý)–·g	ú@isyIm?ïÿˆ@«Áº¿èÑ–8W¿ÔâÜʶ¿êáôÃIk¿ç2Àç¼<\¿ïÿõž}.)AGNbcu3FGL J1045.5-2335NVSS J104603-232855?ìèO²ùD®?ψ Ø¨"H?SŽ†Òܵ?R×j}~Þ?¸oHNð ^?ϒž"('D?ïšI¾—?'•Ãârš_?dX8"5™<?hÖ\'$/€?"hŸ'·ê?{àޝžÒº?î¹ÎuOÒ?'Þ̇5G?Ôøù§$Š?UÙÖä?ŸÛ¿²F´{?Žr¡܈¡?ï,zm%†?sÇdœ(?n¨'Œj?Sáá´ºV?–›­i0û]?q§z›è){?ì4ª*D?ÆaÙ¹Å3%?qf›…ü? 8O ÓÔç?½J™×,!F?ÅÁ}cX?îÕÏFñùO?žïzË#×?y˜à†Eƒ?‡Ö _PZ?žßÞýoå"?—4¾Û³?íÙ'ލ¶Ú?œ°ñ'¶$?ˆÊôÀï?‡º:öauÛ?¬;›¬$~?™˜JQAm?î¬B鉜?=–ŽwQ›?s
÷ÖÁèJ?j×ô'ï…!?«³ÜÙèdz?5Β ˆÊAGN4FGL J1046.0+5448¿ïAÇ~6ð5@Kǟfb5À;;u¨ùˆíÀ<ԆðI©—@#·&rZ@u砍©¡?ƝÁ¿@"…4õ?ˆõŸeÉÆ?ún5ZTà,?î'l^YR¿éŠ¼A9[@¿åäÌh"ÿ	¿è¤8>4îõ¿ÉúÙh<¿ïÿÿ&¦³AGNbcu7C 1043+5505?ﺹ} Ð×?}"Í;'Æ?S±Âƒœ?NŠ
g¼?}ÃTÀWÀ?{½É³•?ïE,ìÕ+?•
MŒ½?pbt¶?s‡¢]!î?"V㝐øu?'ÒË~i?î썷/£ÿ?‹=ꦏfß?tv®:ÄW?rG`ÁÊÐ?PÈ­Hò?‰83Ö¤Åz?¸0w[?k£úêA$×?hvW|i	:?UrÓ3å?‡z|ù³?hoée•v@?ï\¸‹.?m´µ?c·t¨,½?_[u¿?'šr r«?Œ?f·?îræÜjl?£Ož–%Ú?v²y¨x/Ã?Ñ
—«n?¥ûC
ãñÁ?¡r|
œÎô?íî:==£$?–´pã×{3?ƒš?}1?,>PãgW?¬Uuªáqs?"vl,žÐ'?îZô\!­¿?ŽÅìq´ï?"2ZvÀ:?z"€G2ûr?¥L­§Ÿj	?Š"šÇ»ÌAGN4FGL J1046.8-2534?í®ÜøF«¿@=Y¦?šIÃÀ: ⴕžÀ<hHí¯›d@!V%–c.?ù½)Î/£?Èpà'ÒU?ʈÈ%ž:@hæŽ>ò"@7]kT¿éD,[Ø¿éýºÀÛ§Ü?͇ìH=o¿Ó—dá6¿Éø–T?È¿é"VœoAGNbll3FGL J1046.9-2531NVSS J104651-253547?ï"o7_,?x'ÏÛh>?[y7ò@é?L¿v‡T}"?‡Ëý,³?w(uºvD?ï»æEÍGO?y:‡…Xæ"?RÍ8¨ù?U™¡&?}YŽâ¿{ù?uà£F~-?ï	ʘƒÞ¶?ˆ	Ѥº®?t	C$Ö?xÄK¾Ù;?™Ä\€R?"·éA¤J?î1=øù?»'¹?hˆ!hWÇ°?Pá¦ìp«?¦"lx­ö?eÓ­µZ?îæÔáˆ
?"ºÒ·8	3?pe06"•?dqì!íã¸?Ÿ#%  ?'q0ã°e¤?ï+u)ye?—+r c4É?fÅßmB^ƒ?q™tJ÷•c?—¸£jÀ͗?•¼w;zª?í¡Þ
ß3#?›Ô•‹E''?'½z 6ê?"Ç‹"Hñ?°™`N·W¡?˜V}FD
†?ì*5[Š?›+t/Ï;í?yÃNšµ?l^•F¤D?½¸ï˜?š…N3ӜAGN4FGL J1047.2-5517¿ïí¢µ}@+ $bµØÀ9Ÿj'E'À;]ûî"‡ê@u¤œ×è@'iߗª¬?Å­W¼w¯?§YÿáÞ=?ܕĢܹ@«ÙK=¿áÏ$Ã-è¿ç–¾¡¿å,¥3Ìá¿çŠü4µê¿ê$¼ãJ½"¿ïú
ÝÿzAGNbcuPMN J1047-5513?ïr4ñë†?…›Âj}Š5?Oµ ^LR?DH'¢•?»¸æ+'«?"dÝ?ííÔJß;(?°ù_³sÿ9?`IDۑâœ?j/dLêÙ?°ƒRuè?°pöJ:/?í|ýCãÆ?Mƒ5¨·?…Ò¼Õå?"4çÛÌe
?±w‰Ä"?›/Œ	¹Y?îç\¯û¨$?}©dº­!?U]¨r•?6¨éð,v? áÒÔIÉ?},PO'¢]?íÛسµÏ…?¥Ü娗¸?^3õ?L?UŽ`—xº?°¨jŽÉnå?¥x9&3›?ëÃieŽ?Á[õ8³/?oÀý—/z?'ăݯšû?Ãîe´öÓ?Áðo¿*£?ë³z¸W†?§µWø[é?•ð­*.Í?ÈHG†@:?¼è˜wo?¤ÍN×mI?ìõãÑ‹?™…ºû¥9?lBŒ{‡E?TMÈޟ=ä?·n͍yê?˜·òÂw*ÑAGN4FGL J1047.7+7238¿î+qØàVl@Dþ<Q‡À9òOƒËÑûÀ<H‡Þ†2µ@¶;ÁÍ@UYΨo?¼grUx?½Y''b?üR¬9¯N@ÍÉæhE?ª)'þþUä?ï_]"Y
¸¿áµ¹À€Ž0¿âö'î½b¿æ?)@k*¿ãþ±·!jAGNbll3FGL J1047.6+7240GB6 J1047+7238?ïòo»œJ?Ha…D²ã–?6f+GŸXx?&½u?N†r?U†ý'îÖÌ?Dw¡E–<?ïÚ5II0\?qcŠ}—¼g?E<×ð%­Ð?PëW&*¼?p=Àdeƒˆ?l"&^L0A?ﺍùÿÐ?rÄ/Õe¹¢?\›Ä©T-?hrÑ1¢¿?{'˜ˆþ?kW}C8k,?ï¸f+7=?]5mZ®o½?h|Öu±Ä?J¡"9ÞH?wŽ5wF?X-‰:zÉü?ïèjqÊ?V³‰ÊŽ˜?Eö	eBýn?6»Ü.…Q}?bqal›?RÔypW¡•?!k_Ÿ?…ÑÔ§_?XÀad3N?b®5ƒ×§Ó?‹Dkh#—ï?ƒ¬r{®q?ïJó»›n?&_:M-Û?b€í±Œë?f>ŽTšÍ¨?ˆ
¯´©?y¥s½÷ý¿?ï?íNޛ'?|i2Åa_ø?Qƒ9â£?g/%x²³º?-õMøÅõ?wž	‹µVAGN4FGL J1047.8-6216?ïí»QÐ,SÀ*~#ûÀ8ŸüuÀ;$ї6èÊ@nâP3@2²|¿n??°ú¥Î\
?²—ºÇ<@Nõ üÐ@ª;£!¿Ì<Õ"oß¿áùbW
-¿çOÒ:Ê×)¿æáÑv¹¿åö8Öá"Å¿ïÿþ½à ¿AGNbcu3FGL J1047.8-6216PMN J1047-6217?ᅢ^Ã?'«~£j?BBK9¿€Š?D˜3>¸¤?}ö*l¤¾È?°ÿˆ¨?îQóÐû8N?ª]¿q.?I•V.k?]AýÄòþÝ?ªzmš½O?ª
–µMO?í¹Ý4+´A?¢-rRM—È?ùµŒT0?Ž‡K?AÔú?¬c¿u©Øà?Ÿ£³?îÉ°±Ÿ[?|€¢æ>ß?qu¢òÈY×?Qâœ
X€d?¡6@"¯›œ?zϳº¼Þ?ï#Šj–e¡?˜e"d	\#?Uéž?QÙ÷Šìÿ±?š>:Y/ð?—³‹":"?ê{	‹O?Âé	'ƒ?aÑþñÕH[?{<Îháqq?Å̓Ž_ C?ÁÖO=¼	l?ìP¡|«»õ?§{ícՙM?–›åޝ'þ?'BñÿýŸÕ?·Óú¡°å?¤rì¯áǕ?ìÏC×g§Ñ?—d¿È,?‹BzßV@?rd9ƹM?¶'˜ã.?•Â´Â€GØAGN4FGL J1047.9+0055¿ßƶKÅ@I:ÀÛ'À:n©ö/yÀ<?µÚBV@@«6$)U@U`"¥?Ãá!¾Ð?©9½;	kd?à½2?î,™@'ûF²Â?ïÀRÀí ¿ç…Þz¿æÊjåQ¿ë°R®"½š¿Ã"úÉ4g¿ïÿ$m'MAGNbcuTXS 1045+011?ïӑ•X?¹þƒþý¡?p'o9&oß?‰gXØ?›DòÚ¾õ?·ò#3\?ï¹õmâ?šÏaMA?Väšî17?dt¯ 1Ø?}P3ÉW	?}(¾-ÙGQ?ï5àø†lŸ?ŒÀáŒ@xh?f2èâæ?kehESé,?–]‹ìõÇ?‹™‹	'Ñ?ïÍt$¿þ?ZÜfl¡a
?K"µÔÅ?<t~ ?v¡²…Œf?X;}A»v?î-B¥¹Z?ÂLøp‹?~Ý+æ»`?'nÂ	ãA?«±†fµ6p?ÀYë›foÃ?ïP¶lŽ?¢Õm+èÁ?^Ч™'Öù?mÁ͛Ðê·?"~¹‹ªØ?¡'õw§0¥?îMQyfÀ¡?˜@éUùĘ?zڗQr?{ÃC;´ü?§èí}̳?–Q&=ud-?ïUTé™ê«?zÍçQü؞?gqŠ…Q9?_Ɗc³ª?'g1zfò?x•IÁÕ£çAGN4FGL J1047.9-3738?àÜ^ËÅïA@3*ýڋÒÀ:ÛCîlYÅÀ<ˆU|3WE@!"':ûSž?û9JÚåª?Æ*ñÛ¥Ø?¹ûOìýD?öâý¹÷@îA~5»¿ïýš?[à|?ïáäVVMê¿ÛÚ胿¼ŸXö;¿âd.þ›&¿Ým ßôq×AGNbcu3FGL J1047.8-3737GALEXASC J104756.99-373730.1?ïÜLt?\¦AؗM?;jˆ:"p?&°t‰59›?p#JP9âý?[L€k03Ô?ï҉êqoÑ?v¹p&i-d?NÀQB'.L?X…ƒá™1?rã}ÄÊ÷?r‹a·óÔP?»B-C?x2ùÛ°`Í?[éíœ^››?ENPɲÃ7?Š ÓoŠC¿?w¦ނÏw?ï7Ÿãy{[?pê0W?r&Èñí?RsæÂB`r?"'QL¥i?lj†~èö?ïǏdâX?iå†û?F°=ë­?4ÏlL~Åu?y¢°Ÿ¿W?h°É'è;?ï…Tï¤?ŒiôŸÖrß?_mÆh?ë?jÙW5Ð(B?ŠÍñîwõã?ˆáŽX{tÉ?ï*Ҝ'é?ƒ
:@@«x?dßtꗞÒ?VÕ a. (?˜!W¶f?'–· Ãj?î-s/™íõ?ˆ'çR>y(?'6hDe?l&^ÀS…?¨›Hìê	Û?†Ïò/ؖÍAGN4FGL J1048.0-1912¿îÔÛA.Él@Al½QðÀ:ùíp±CÀ<ƒCË0ëZ@†8sŽíï@ÞõfI
5?Ì}º•èŠ?À€È|)F?ñCâtÔ¾?û0£0œ*?ïÿì»"¿ÛÆDóO¿éÇ :ˆ¿ä/9ÿU5<¿ã¦ YžØ¿ïÿÿ" 5•AGNfsrqPKS 1045-18?ïtg§?ZÅ?´þ
²Q>?W'ù°^s?SùÌð´Y?õ·	"'õ?·$å±?ï$ïÅí'?"J¤ùq?€\žèÁ%¡?}ðJ¸Y$?•M"'¨ñ?‰w•_d?íµF©Éô? ©lãgŸË?ƒˆ…ņB^?ƒqº ®ðq?¯Ésûö1?Ÿ;ûͤ	Ë?î•æßÑ
?‹(ÎdQ?‹5[5î"í?oåúÄÏvÏ?Ÿ¨vqÅkå?x'S'·Ç¿?ïˆ{[g?™»{&øù?iéހ&t•?{È;•º?šñ´Äµ"?—쩽ÒS·?í´À0îF?®³/¨ö??'ý5xÇaà?¡%ÿº}l?«?¹=κ?£¶³^¢ß?ì¼NõRõ=?¥'t™l?h;gQ8?‹­"‹-i?¶yu ŽL?¤Y(…ó.?ëç¼Á€­(?—ö&|/j@?¡Ó*·s%:?‹´ïHhG¿?·Ø"™ŠÞž?"š?ôaNAGN4FGL J1048.4+7143¿íûqºFQ7@E$	_$RÆÀ7"
ƒÁÀ;4òtý@/öU²9#@ ;>šo'?ÈîN…QÂ?µÂ¡"~–@&0¼Y¸:@!áªqKµ¿ïÿÚáb†¿ê[y£Z¼?ïî.¡©¡?ۜ@]=Gß¿àLZK¥ñ¿É¢
cAïAGNFSRQ3FGL J1048.4+7144S5 1044+71?ïIpãS2=?°£á‡t?uÊ¥3l?"³i"¸h?'_:M-Û0?¬Ë°Û?ïŠfIFV7?¤–nˆG,|?a'r6û\?vUY+rþ?‰,l'm?¤Ñö?ë÷ ìº?§‰}F)?ªöˆOGÐt? ;š‹·!Î?²ËºïxÊ÷?¢<Íà¤ï.?ïüSBû°Ä?<"ƒõèëq?W+äü€Ø?vAÉ¿?;l¾ ?;9ã›	&ë?ï™EaðB?®"î-÷]e?Y˜E
^a?"ò
«b?†{¥ÆVC·?ª7‰ùÑXF?ÑYW?·ËŠ":†™?ƒý•YPxÈ?¬=\\ñIc?¡^àïêØ?²*àI‡<?ì|;™V?¦«3´ˆ>p?¥Œòç¨h?Ÿ;s®çŠ?±W­'º#?¡PpÓ?ïö¥ïú_"?Tžs¼óãR?#L3×þ׺?3i,'°Å?PJ™Lè¦Ó?ScþQ\žAGN4FGL J1049.5+1548¿äÎXGa4ñ@MÉrGE8ïÀ9ï`sÞ.À<_þ99@I6ù;jº@$ù´Œ?¹äÖÙÀü	?¶‡ÑßÊð?úd§՟Ú@V'+áÛ'¿ä­òˆH8¿äJúú¿àc^Caÿ¿ãmó=yÞ¿ê´RbM}¿ßä«üƊAGNbll3FGL J1049.7+1548GB6 J1049+1548?¡x$?{Ãí
FZ?kÞ{[Ð>?['ÀöË?‡ex¿TJL?x
âȾ˄?ï™w\¡?ƒÇ)4*μ?fĚ­Ï‰P?p˜CŒ&~l?ƒîû›K[W?{ÒÝ¢"û;?ï(®¬?'w?Á%m±?zKbê/'?ó\ü(Þ²?"WQ̃Œ?‰6º:ô©¨?ï"¼7(G?tÞ6K@C?…dKþË?e<tv?öY‡
F?o€¼"?î¶åŠ2ôI?–ÛG|»Þ?"´œä®"?vµ»F¾.'?žÉIúÍ?"];GéH?îæÙ <Bs?çûɱܩ?x‹Æe14?ƒ°-*Ì®?Ú[çÄ?˜H©¡€l?îM=Q	™?™n`»­U?‹I# ÿ~?‡Õᄰ?¤Yß$«??"¨Tô?í¤Ølñ£y?'î3ʓÕ?œJ_\í?''Œ2s‡Ç?§I­‡²ó?‹¸MߒêVAGN4FGL J1049.7+5011¿í¨§œš2¤@L¨6m
JÀ:îÂfA}yÀ<Õ? §?u@圧k@ÂeŽÐ?É7ôãí$Ü?ΏH\æ
?þJ†_¡P@é¶H¦âØ?îrò yI¿ãÊ\º³¿àd¸aý–¿æMzV[V¿ëoýV'n?Åb¸ÜÕÙfAGNbllNVSS J104857+500943?ï"OÌ
?€ùÌhݑÒ?kÝã*žB'?aÆÅê§â?"ÀèD¤Ù?{Å2
50?ïy<bJ½?…:n'!6?iN>ê[?jwúh¶³?‹H¡ç?*x±8
?ï$KL7CÂ?©Îíyų?wå,"3Q?xŽåB[5?•}K_mÜy?‹º-]½<º?ï|¢ìÆî?hQ<-ŽË¹?xJä0]—?XOOQهâ?"²Dq…9¡?cš!­x´?îIJ½Ui?"l˜\‰—?'¡_Ʉ¼ê?vÝr(åc?žþ!Û&j?'5
ÚÁ°y?îËø'ÅÈ?™.·,4c?v‰MT«´?}xU¡ÿ? oTt?•IUYYÖ?îK}5&?˜³³\?"t*´ìV?'ìB?ÿ?¦+":ð?•`:%¶`?î^ð‹mÜÒ?‰œýnƒ«?cø¹>ïb?t×Ít¦Ú?¢7ùŠE?†Ò!ãdAGN4FGL J1049.8+1429¿²‰äÚÈ~ƒ@M'bS—WÀ9LwH5ù·À<2¾Ÿã_¶@q*EÎÁD@kÉÚª"?®žˆýÑ7Ò?²=ïN×Ôh@K¡F6E6@Ê
¥/$¿l{É:Ç¿ä«QݘL¿æ¯Õ`EK¿éœÀË6ʗ¿ð?ïþËÌÍAGNbcu3FGL J1049.8+1425MG1 J104945+1429?ï÷®UpþN?Eºv'ٖã?8²ßQ0?0ÍüKPµç?E;ї:iþ?A¤*` ?ï»RQq?†¸{é-?[õëŠ*?zɬˆî?{Y'¸¿Ò¦?xŒH-¯Pf?ï{(pȦ3?†ZH¸åì?±nÓ?~?ƒ|õËPýE?²‹
;¢?xŽàtöªG?ïévM=d?J=õT?TЛ´2|?@x#D?XC5Y]$W?@"¼H¨v?ïðkGÞL?XÙí0l?F¤@Ê÷?H'Jáՙ>?T$klz©?Sëªæüy?ï@9&Dì?™ù(ã]ŽÐ?lï™Ê¦µÂ?‰±YÅ<ae?"Pš×XØ?'KÝÛK~?ï+™DùÈó?žíâX?ƒ`†c¸?‡×bÿˆô¡?Ü×ñŒ¡?ƒÿL‰@ ?ï³K'£Öß?q;Ï©h÷?rK÷­Ô—¥?e}ì̒Üc?t?, ?cÂêÙѺÂAGN4FGL J1050.1+0432?ëþ{'Ï @J¨Ü]cˆfÀ9UóU͒À<,	óžÉ@Yø6zæ@uƒž?°‡ÇŸ'UR?³óÛÚ[×?þœÃk$;@£3ž¿Ý%#:—«ƒ¿åâ1ž½d¿æwKüWÔÓ¿ê\ÞCÖ¿çŽR"_¿ïþ‹ Z›AGNfsrq3FGL J1050.4+0435MG1 J105009+0433?ïúíE?2zv!3‹Ÿ?!—&Ù·i?ç¿ÜÞe›??ÖÔðƌ:?/©"''…y?ïàÈȎØ(?iœ8ÆH5è??Iì£Éç?L•÷'c?kMú}÷Š?eµ7_µÃ¬?ï¹Ômçp?q=ï(\4?X¸±W;~C?]@%4nþÛ?|眝4LÆ?mþYDéa?ïû'+!}?%¡T¸Õ<­?%š3Àÿ?ÎÜZk(?8ßÙ&þ z?!Dü"Éäæ?ï÷üPüzm?Bß^+ý²d?''ˆEÃ:P?	hÇf?JDÙ
Àþ‹?AP¨šEû?ï¡s@¥Å?"H,fÕ¿í?PQ§k‰Û§?\,~s°tO?…˜úæ¥5æ?'}rHQ:v?ï"Ól¼?~u›òì?dg°'…&?c‰æÈ°£?‹ñF%i¡?{¤‡SYåî?ïô?Àà0?Fhó•Øª?>òúC%1?2cú<4‰?PBÁr~(n?@úèN4$AGN4FGL J1051.2-6517¿Ê/1¯-2FÀ0¹~;oBÀ9l™ÝŒ7±À;·ÊX~F@"ýûÃÛ7@ÛØ{V¸s?´£è}ˆk?ªœ©!)£ñ?ô‹'æÎ×?ô
ôÀéú¿Ò.žÎ⧿Ö*èÁŸòú¿çм{Eñ|¿å¸/A8¿á¥Æ}þ2 ¿è"ó!uE§AGNbcu3FGL J1051.5-6517PKS 1049-650?éRQÁ"³§?¹È‰'±7?x2JÊ8{Ò?yœN :°E?Éõ&¤Øæ?¹£ÓªóšR?áRm"?ÄèsyýÑ?˜þs…U?"´e
P¡?ÛÚµd©h?â#ÐÄ?é@=]?®1³ÙÆ6Y?—tœî?ŠYµžŸø4?È[vb Ë?­I†£öÿK?ç_ÔÅ·? 'Ôäc;?±Ýgy0Ï?Ž´óAt¢?ɕeø']=?›ÈéW5à¦?äBX7#­¯?ÀåèTñ?‡Ýö	Ì[?*°›,?Ö¼_áUߟ?ÀôÿÆÊ)Y?Ït)ÛÏ&Í?î‡êgð?¦ÛÓ?¬ƒŠ¼2?æÁeXz?Ĉ-éûº?ä&56œÓ?³"CƒÚ¸?¡ìD¼f…î?Ž[‡ÛÄ?ÕvI˜?²´à®¢E?ÝéÚ3…?¬Äuð"þP?ÃkíR?¥
õ¶×Á=?ؒpmÙÕÒ?¬DJmó‰¶MIXED4FGL J1051.4-3139?½$ùšÇRK@8¡¢¤Û<À:žpÆ;¹À<OÚy]¹ï@ÿ·1Ô@LaÿÏ?Þ'_Tú-X?ïü«ë«µ@ BÛ@ í‹^B¿à‹ÛÀÛ|é¿æ(bÙ	¿ìÓ¤¢š¿è9ê™w5¿ÀÄbÛlwÍ¿àöÿ¦=ìËAGNfsrqPKS 1048-313?ïWŸ/þU?•¼lÓ?~˜®(.n?³—1¸qe?ŠËÝ5;%d?3Ô'̝?íëñ]ÙX?½s)¶e_ß?«üÇ'¦ ?¶•¯+s˜ ?¢yÃW±?¤ÆH¹­5X?íßkØ7±?¢ÙÜþé‹?W"ñ¬-°?–ã0pz?°K¥¯?Ÿö~íˆé?î2
".? G
PÐð?¥Z'ªÛ.'?›
ß¡¹Ì?"g"oÖU ?‰Cé71]?îàØ©žÓ?¥ÌÞ[é«m?•é÷¢[?™¬«Xٖý?¡¼Hˆ>"?—H!ýŒÐa?åð¤Û…ç?тëï_@?Ì×"UVf?Ðdn Wß÷?¶Ðî,‰o?´6"	Z3ã?ì);ü8'í?¥Õ› ¯s?£U~on8?™f5<m†¦?µ4u\áGý? ¸æ\ˆ©?ã4kzCà?È2iT
!?ÓvD™§?ȟi–‹a?º?VËzb?´_eóeBAGN4FGL J1051.4+3942¿èe±s½@OS?B5/À:Ò ùtÌÀ<'Ejm\$@!&Ö>°!?ù•¸~a.ï?Ä®j·ù?¼x`äÇ??úa…Æ}þ@B·¼Dif?ï÷"ÁpME¿è!œÓ	ý°?ƐöGo€A¿ä‰6?W-ä?±Ú, ‹À¿Ú"þPÅAGNbll3FGL J1051.4+3941RBS 0909?ï«R"P{²?'$šîs/¶?E­Æ­oØ?<
́I''?ƒÐšù÷@~?±Œò·€?ï¶è"Ø`î?}úH÷Úë?Q¶g"^­e?W/§iGZ?€*R¬z¾?z_ùÝu•D?ºó3?–Uû©?]‹]û¸?ivɛãI?£_ó?–tÉ(ô*?ïPO*à~Z?tø[,f€?M&¬}ü?<¿Œ` ?•å>ÿ1]?tÑ›c}?ï*«ÿg1?'øNI¨ÚC?ZÖ§D'¥?Pbì\ª½é?™¢YêS²?'"3öhä?ïF²!Xræ?—ÝYc¡û?]"•J7XG?eaG·‡gÔ?•W'ƒ½É¬?–"…MØ??íbúìÎR'?¢åúÇ5Ì?bՋÀƍ?jR)5Šþ°?´W1îL??¢É‰
%(÷?íµ¯yÕ¯?—Oö"D»´?`1'ñM@k?WB^u|¥?±hÅôzí…?—z­ŽAGN4FGL J1051.6+2109?×1HîT@O
üçFÌÀ:Œ@O{hVÀ<Z)ôÆ@èåtc+?ýy*GÒ'?ÚÉLÅUŠ ?îâÁ*Øß@ã*!;¹ê@´ÏüØ`¿è³pÛ4n¿â.	È֞¿êqN õC¿ï£GÞ#¿ïLZUÕõ¿ënƒÁ@&·AGNfsrqOL 282?ëÿ͊YW,?Ã^‰h=Æ?U¤K¬¤?\ö"Q*	?¿«zBU)?ÃN-ŽÈI?ï
À×Í?§éUë*A-?‰v8NLªƒ?¡¸ey»ß"?'ŒÒI÷?"þünú?ìĚß>êL?¥7ܑñŸ?'¥úµo6d?Œ\¥™îXW?µ1ªX¬à
?¤ê*üd?ï@fî)F~?:Xûˑ.?{óˆ3Næµ?n#¤]Œ‰ü?ö@*ëЙ?|™ÓQQ{{?ígÂm3›?»
 •K×?cÿ.Ùè*U?l@âÊæ?¶ÌÈuC0Ô?ºÂøZº?íPˆ
€C?¿vHj.¦?žsκŒÊ?²•oºäG?«½˜$Åg?´k\©h•?ë›þfݖ?ª??k[àÕ?•‰´·;ÇÖ?'+,·?³?½½¢žŒ-Ü?¨ŸÐÆ+ž?îZwwÛ®½?™­Ä†Èª«?…Ê›¼€ñ¤?ƒ¦)n¿ˆ?¤åá'HðÉ?–È2I¬±AGN4FGL J1051.9+0103?ÛfÄ|"œ@I¢pÁ3;—À:¨ÓÚGóÀ<zµ'»@ "~/Zá?ûÔ¶:º2?Éž–Xœy?ÊÁG3@nÙ8@ Þò¿%¿î^&@Üi"¿Â'Š^h@0¿ÔHÀc1þ€¿¶[Ø}Z¿ì\'Á3¤?ÀÅ`‡TG«AGNbll3FGL J1051.8+0105NVSS J105151+010312?ïZ±-xÍá?ƒ<mF¼ìG?r½UɅ?g6*æ0ìŸ?õ
#\Š÷?­Y°nžù?ᄊJÄ
O?y>Õ'l?X†íxÇÈ?aâ}ÿ+d?zƒ7"›&]?sÛì²À¼?îð6¬Âôº?'|Ž'•Î?îIÚ¡š?€ýpæíi?™'«ž?ÃE+ܑa?ï&ü`v–?s4Ì¢ôÎ×?x¹$c–?^($,tC?"ù?cƍ"?oÁ}Œ;mÚ?î¸Ý¯Ñœô?•Pܺ¡>8?'ã®Ɋ?w¨9ŒÂm?ŸÝØ&¶çÍ?'ùÝ^çØF?ï5°'Ð?•ÿŸA€&L?nÔÎJ9®?y¾Gx5ƒ?•™¤Rñn·?'´0¯ÜbR?î$"ào¿?˜ÉŽ4þ½Ê?Š£Ñ…?…gFc¦=x?§8)²™r?"ÌÝKœ¡ç?íÅj:äàó?ñðÊbLA?Œ'…«u?ywŸUé"?¬"Ø1"ðl?ÕSm¶úAGN4FGL J1052.3+0818¿åáKŃàÓ@L.‹*kÀ;(Ï,"žÀ<€w˜½Ñ‡@éª{i,ê@‰$y\p?ÉÔ®ƒ
¶è?ŠÉ'"C
?¼"•£Àº@>%ühñ±?Á©p¨	¿éº¼"pdí¿Ù·áéÏ¿êÉÞÛÃ
¿Äpjá C'¿ïÜè‹+BAGNbcu3FGL J1052.0+08162MASX J10522451+0814095?ïÏà]Mc
?rÁ"ÚÚÞ?Ax»ñ¶þ?8@åñéF?uà¹Ó¹Ë?qì°/ÊÆ?ïÂÝù×A?'|ä ‹CË?J-,Ä=î?UÆG½ ^?{KbŽõK?!7'd?ïLÀ_×,?…?o)ú?eUŸòQ?p—Š-;à?"ÇIVë\ ?'ü…ý{…x?ï֔7k7m?S=z·9¾A?3H$ä!ùô?"¼³¹Éd¯?sb»"?R¸°™CÀ?ïf^šP^ù?‰~Ë»irì?Tߨoiª?R1ž{0C?'æ;D
G?ˆakÛ¬Ò?ï-:yV?ªgÞoŒñ?Y˜ë¤¡[?ijJÖ>?˜Å¯æÑÊ|?ªD"À­(?î},Å0T?"ìûC?p~¹#Ž®¼?v÷žc?¦\ˆ`ç?'?aÚ÷?ïs§Ï^ÄÔ?vóŸ¶Êp?KØÏDFø'?C¥ÃJ)8?¬?˜Ú?vtà˜)Ù£AGN4FGL J1052.9-3743¿Ù/Ÿ°4Ò@3r§›ºÜ
À:ŒPx¾W¿À<|ÏÓèJ@ U*Ï?ÿI¦Wíþ?Áå'Ác?°JCp?7?óec>"º@,ŽTÁù4?íº|CG}¿ÀßsXd¿äµ¿Ý…*¡¿,ü¿Ð?›PÔ¿ë.
ß¼"šAGNbll3FGL J1052.8-3741PMN J1053-3743?ï½ ò©UN?q¤µFhX?[hVS:d?g«àÿÝâ?zL,'>=?g?ûDcÅ?ïª#Mž)²?â"O¥Z?Wy$֏so?[4cR]b?'ˆí}{?|f£r0?ïp@zŸß?Å•®£¹?bÏh_ô2?izsCX—3?<U$mÊ?€†ÿ¤«î?ï+öÎ}üÛ?qH‰¾P¤[?p֏ÂuóÝ?SCJì,e?–K'G^?pÒò#öÃ?ïnº¾'â?€u&='?nW(0üÇC?dаyµn¦?Œ»†y7k«?{Ø¥|]"ø?ï*Ø\^5ü?•IÒÍeû'?dmê]'3¤?kXžó"?˜7%Çj?"-2Ðþ-ð?îóª?ˆkô'A?m+¦Åþ²?k`5kçð˜?ü˜sR'Ø?†ï)'«"?í'kyíú?$BÕ´?†»ýÀ·J?r¦žž"äÜ?°$vÁx<?ŒxN²k‡AGN4FGL J1053.7+4930¿ïÿä#«€Í@MEhÀ:´ñä´JÀ<m¶
éh@nˆcf?þ/}0­Fö?²ë¯α?žn"h¶?ìܲÞd#ì@.ø3
ò?' Wú?Ê
áÄÚ¿âd…†"¿Ýýc˜€À¿ä&@×`¥?º>¤@¼;AGNbll3FGL J1053.7+4929GB6 J1053+4930?ïÊ'ôï3]?qó+³óo?Fß
œ*ë0?;œà•)×]?x$?qA4ӜIÍ?ïÊuURÓô?w˜˜u¦?RoÄKh?Z™O¥
bC?v?yUÁÿp?r"6ÿó/?ï'ñ;Ÿ›ð?'»õŒ,Ë?q«_?"½þ?€SêVÙ':?–—À¢Ðƒ?,$ƒêq(?ïmÇ:*?jÛëî?wÞ&ü˜]?Z5`u
Û¤?ˆŸð‰s?d»;¶'¯r?ïÙLJ®?£
º ÖB?VŽ.[¦ý'?O¡waÁ]?‰7ÈF¿ÒÊ?Œ°ÉùÜS?ïhüµ?î…‹;?`ƒi\µ¤?hKÊ-1"Ï?í3I®tÈ?Œd]Ýu?î'1ƒ¹;(?î®¼.÷?j	CŒ¥÷í?tøñ®,s?¥<SŒQÙþ?‰ûšTOo?î~ñԇðé?†»ORÌÌ9?Ž\
ilwš?tðíà!«? yß_¹ˆ~?Ê'ê¾ÇFAGN4FGL J1053.9+8628?çÑàAF@>0)à¤&À;7Žd²1@À<Œ†ÿc"@ =ºßd@W#"ú?ÆN­øvHÝ¿ˆGQ€Ù·Ê?Á<×xLm@(W$T9¿ïwWÂHå?í	ۂr¿ëx¤ Üš¿×ë'D"Wá¿Ï
W–꽤¿á#=Qš&‡AGNbcuWN B1046.1+8645?ïNU´,?£Ú£æ`ƒ?V"cç?N€¸;§ƒ¨?"Ó±=[G}?£¾Ž­?ïÙ""¿?m_ÒÄÏ¥Š?AƒÍî͋?Li_­ªô?q>tù´ÞÛ?i@–goÙ·?ïØKþR£?ŒkÖy4?gYbí?ÿ?i½'ø-|?š¹Ê¶r'?‹B£ÀCd?½gK‹?c‰Ü0Ç
?XæŒMkÉ?Eb+XESÙ?ƒû ÷8]?c	¹)g?¯^¡?¡c
U"þ$?k¿þ¿°Ô?d–þ¯'b?¥I$=ûLã? ÄÒt¯éã?ï‹Öiry3?‡LÞÚ¥Ú?V¹äÚ4c?aڞÿ'=?Š3(ú´·c?"¼Î€jÄP?î€;	sú¬?'c÷¤¦bâ?p9²{*TP?p"hX+¬«?¥õTÑ0?'LÂmð?îä5½.Ò¯?"Ûw×ÊN?sw¹Åhm?g¥ÿL‰˜?ž›Yï&í>?'ñ¼¡€ ©AGN4FGL J1054.2+3926¿ìp4c	Ç@O`ïܜM©À;Ê;"À<±ákÀB{@&a"ðh@h·¼šO¢?Ô	éã³ï?Ø*Ov`@ÇMœk2@J‰äDãŠ?ïì,CTéf?á£ÂýÁy¿â° ¬³R¿äiêIµU¸¿ïü`¾†¸ì¿é'kb#¶"AGNbcuCRATES J105433+392803?ï®År1î?‰9V\:æ?€'v¾«}n?s8£
s?•ëóï‡?"7/
¬}?í#¹¡)Ž?²SðMµ‰r?§¯¨Êpo?¬Üñp
Î?¨˜é™­?wì…*Ë?í¸=²yJ«?›pùºß4?™p•ï_?W o®†?§ñlãAÍ?"ŠeI/ôº?ëuHMîî?›ª(IßÃ?·æOև)¸?˜h¹w¼l?®LÎ?Š1ózÞ?í˜"Ë~eƒ?¡K](R™%?–æŸ]ˆ.S?ŒtvN¯É-?«
ƒ™U¦?œÇ²4.֎?éÜ*2ƒŠä?¿FG™éíç?¶("ÇîXÈ?´vô<΢?ºö¢='?´ä2‰F
¡?ëÿà)Ã?R?¤F1Íäl)?¤Q…y"Â?"'˜XùVÉ?µØ}mq¦?ŸàSÝì|?æD«JF?¯<Ekõš?ÄUb—Ån?¯‰€ÖUìÙ?šz»Ä"?£Ybþä!AGN4FGL J1054.5+2211¿ïf¹r|õ@O…" ä¶À9s€*]À<ò³ç#@,4XÍ@¼{ٕ2,?©?Ï£Á»¢?§S›2 ç?ü½CŠU@ÕàòŸ?ïû)×iß¿áón!EÊå¿â88 þ¿áI™;¥È|¿ä5D௭­¿äáü>ª_ºAGNbll3FGL J1054.5+221087GB 105148.6+222705?ïìµ
χ£?TôÓ/t-@?9ÑÉl‹:§?,ÿ´Våß?`¸Áža¨?RiŒÙ">í?ﵩ7ÏØ£?|¤›¦rC·?Zksà?cí2GûÂ.?~œ-'FS?v-ÒÖÎ?ï½géb›?pL3Ž½"?R"Èˏ Ì?=å c¦XE?|ªÙMº6?p "Ü?ïjÎäeV?qŠ†"‹+?~7˜sWÿ.?bƒ®Mî8ð?†0z¹]?g˜kÕ9Ѐ?ïÛ#"?c'a×??Hã̄$úó?;ì+GԚ?n¨Óý%*?ajuÔíQ'?ï:¼âI
á?"¬µ8;I?h£¿¦v?r`ýï£??•"Yju,?'¹ôëÀQ?ï"#c!?z.wÞ.·?]iáºTƒ?\"å&e½p?‡Z
žI?xn4'Ž?îôŽ?ŒMÂÅPÆ[?"­šE‹?}í%Ɇ?œoCdı?ƒ0s(T…AGN4FGL J1055.5-0125¿ë¥0_)—d@I
ÅÁ?ÐÐÀ:G­§m—³À<OÏôŸy­@ >è{~ü_?ÿ‡ÚTtÌ?º›äbÈ¿ŸZ|Î1Ñ´?ä¥	Œ³@@"¯Ò–¿Ãòæ&¨¿ëù@€¿ÇK	ÿ\–¿Þ|_p#¿áb¡ N>§¿½@Y6}©AGNbllRX J1055.5-0126?ï¶XÎg…?zºÁ‹;å	?WÁM²LXG?F?ƒÀ‡º?~ãEXPƒc?yë•>?ï«)"D?qWéT¨?WaØ3ɋC?ZN6?'Oz•^'Ô?€ع«º?ïjbrÍ
K?{¢Ë½ÊM±?b²Z'ÿ?[žÇkçí(?]fQ\'Ò?z™M•µÚ?îܘ2¶"?uƒ3¾Uá?pÉÚ«¼ï¦?QêC9€Ã? ;Ô[PM?tó$"ï?ïW×À¤S?"P0º½–?kè£Ã@=|?\»ú?=Vô?'‡óvQ7x?'Y×# =­?ï%àܛ™?ž]&–?eq¹ÀPs¨?n³ÓÎ<?œm¨ûh?œ½½s,ž?îƍ½K?‹O퍓z?p•ƒàøT?oS*•oi?¡‹f¾	—W?‰Dr'òõü?ì±»ª™?"÷ ñ,̓?…r"×ýIÆ?p´V{-Û?·Èç¨lÜ|?"}wü›AGN4FGL J1056.0+0253¿àT›
»xo@J£þ¬BêÀ;–(Ÿ~¶À<­¸6<Òï@#U´D•±-?÷UGZ1¥?Ð[j‰á•²?«™lÈ?Þ6B\Eü?ý¹U̐<?ë~·–ã?"(H7k?íjcì8¢ß?Ôìi ,°¸¿Ýê!;¹êr?Z9¡%BôAGNbllRX J1056.1+0252?ïٝ;ÿNn?cΑñ-Å?5@1"O?$æØ*êµy?qÝ^ùR?c)Bnº?戀.z«‡?"[_ˆ7Z?Yèúúåhj?cô¯þj"?ƒÕ÷1=?z-ÔÊ?ï.ۊ™?—Çh|¿?^–ØJ4¦®?N?Óaâq?˜UwÅâ?C"¡¯Š?î74
'?'·µŸšË¯?lÙ@ø¿?\±ª]êGƒ?­:Ï.²ã?'Vq«ÝÌ¡?ïÂwão?pÖÕÿ™Z\?=£9À¸r?1T"ñav¦?}#¾3t|?pYƒ£í—?ï{÷>²»?žc_>âo?i4vdÃF?u£+IÍ?›ÉòS¤TÏ?›`6‡·«?îÀNTªYä?'ˆn'Jn?e†º
<\‡?]½¿F?¢¢¯Sw?'-î¨Q´?ëÐEaÅ?­ULb¯!Á?~0än?~?XžìX?¿> 4úo?­&¬8ÃðúAGN4FGL J1056.8+7012¿ä"ø| [ø@EôÚ<÷À9,azn['À:§9zu$@TdhµK&@Y£ÙŽ|?¿¯Ý'ãɾ?½*Œªü@	Ì΢âa@ÑD]'""?ؗ,¢z¿áø"»ìª¹¿è³Œdþ¿èžaŸ­.ø¿ìa‡"à¿ïý¥ýÖ.AGNfsrq3FGL J1058.1+7010S5 1053+70?ïÉÉïð	à?u‡üM—Ý2?\/íÜ<°?`·ÿÌۑ?tB»UôÜ?q>zÓʆ»?ïÏç^üî0?wñín´ê?O¹‹—Ï"?`ú֎*D^?t+ÙDxٜ?rMñKÆuÅ?è³a)CMæ?²M/B¬°Ÿ?¥Ù+Ó3|?ž[|I÷?Ǽ0eÉ?°>7ô{!?퓤ô°Zj?˜ÁÔ㕰?\æw5ÌJ?H‹ÖÞ;KK?²ï>|ª…?˜^Ík"_?ï?•Ðx?œôAc€5£?sSxdvf?˜‡"m.*?"8gÚŸF?Ž_…«i?ïoÈ ¯fÏ?jŽÓ½¸Ð?`g×5Μ?sã9ï…?ÎçqMQ?Œ'yÝà?é…ÞuZŽÜ?°7†ò%‹{? ¼äe"?—[²ªÍú?Ź²Xhˆ?¯AîÐÂJŸ?èÚ\UIH?³Ênÿô?wrm«SÔ?gˆë3…?ËÚþoBiB?³¥[ï"øËAGN4FGL J1057.2+5510?é?'ì
Þ3@K"£½ßÊÀ;7='¨»À<á±¾SF@!-ÒK;é?óT5€ëM?ã9û¤P­?יG¤¯L^?û"üa'@˪ZÜð[¿íÂÎ{ùu¢?ä?°¿í#è§ô¦0?ÝWH…Ö¿Û'îM®ß¿êP
¤ž°ZAGNbcuSDSS J105707.47+551032.2?ïÓì ø?vTW¤»c~?BŸ`z¸†°??·Î¥ñ?sµÓmÇ?u‡+Ã~J®?ïàmBp	u?j°úI_×ð?<""z&?F&ïò{´?lêÂJϜ?gxºki7)?ïOHí?‡ù-Q< ª?fRŒÓW<g?oƒöX…&ï?"L«¨…‡Î?†'"'¸Ç?ïàom'÷?T¦·Òþ4?;ɲšà?2ÎÔ@ÒN?lHk6ˆ?SÏäÑõ¯[?ïÍ×oȌ?rÐõä'?LZDOù}S?KôÙÖÅ7?uˆÿö¡X¿?pG°["?ïœ,H¨?‡ÇeQ4óI?QIJ"Æ?Z¹'xƒßõ?†ËѸ	•W?†J­CÊP?îá,ŸèŠ?'½šAï•x?kG;Ÿ.¬*?q«Û=ʄ? 8ÂFê}À?'iJÏå?ïÅKŠS;Í?m(Óþ®=?Aj¤ÉœÞº?P/Û¤öü?{,æJɾ*?jóЌìØFAGN4FGL J1057.3-2341¿³1öÔ$ˆ@@ó.ZÀ9ã3cښìÀ<PÕ˨à@+³ß•ý-@SEø1Õ?»Ñá߃ˆ¶?ϙ‹Và·@r:½k/ú@Ü¥!âþ½¿ØHˆÚځ–¿Ú¬Cà‡¿äû…LXž¿é¼­?"¾¹¿é?#âqŽ¿ïÿס<%JAGNfsrq3FGL J1057.3-2341PKS B1054-234?ïwB‰3è1?Žg°=uˆ?{€æeiW-?|V§Sƒò&?"nê|?ƒo½8r?ï£|Žü?ß™òj˜?fÌyóèkÎ?k·Óäº?m½TØ(?xu$ÏØð?py¹?ƒP\¹g]é?lRûåf8?qRXv"w?ˆ<äçê˜6? Ô·¬ó÷?ïX-ýØø?mD-0?'¿|‰ÀÁý?aqÊUÍ´£?‡5؍ô?bárA?ú?íî'›ýø?«^dÒ=?šÞŠ¶éí?›ÆKÛÿ?£®I.;4†?¡ŠÂ}rÚY?îöD3ò`?™r]^¦ˆ?|KD¯á?"²:A«õ?š2¦Úðˆ?"j¿¬÷Ç?îå&,åfL?'x%Û¥»c?'…,G?Deäü
–?š¤Z ‡
?Ž{¨'?î?mµ~ì3?‹`5»œÐ?™:" øYT?v%ÄàB>?žØ'+º"P?Ùåá/(6AGN4FGL J1057.8-2754¿á)'õ	@<•ŸÓo~=À9ùhG6‰À<BÃú–3´@ }'Ñ#I?ý"VÁ­´Ú?¸cfAR…´?®3Øþ?ö"æ™ýl¨@ WمÂÍ?ÑÀ&€ó/¿Þ=¡`¸Q–¿ß³þ4Måf¿ÒõJd¨ E¿æõ2F¤)@¿«ÀÀ9ÁAGNbll3FGL J1057.6-2754RX J1057.8-2753?ïèw½ü¥X?U¿©AáÛ?>õUŒ>9?/ù«ÂÕò?c©—²K+?RÃ[Ý¿ð?ïÑéÁ?t‡ìÜ9?MK%A†¦‹?W¯".¶qK?saºíí§å?pN"Ÿ0b?ï®àGuVç?qB¥˜]µå?V8EÓá'?Tã'rVÔä?€å]ßN›?p8üMQm4?ï4^'8å5?k)¡Bg$?r%ô£+ò?OY0L€ ?"óñ–ëi?h ÒZÐ@?ïÚO¯ô,–?a·£ÁJî}?LTW¤j?;¢f/lí?n›:F`1?^ó¨å¯Q?ï|érþWè?‰ìB
Â?aÀؼ'?iÜ"»KÝ?ŒUm1ì6?…¶·œè?ïlоT?}`G[(?`Ú ›ù"°?Yb^#^ÅV?J¤&÷?{/|é¹X?íèêË̂á?…Úúø¿?†?ñ½t7?fÎþ˜[\ñ?«ábR|ñæ?"lÀ\£ÝQAGN4FGL J1058.0+4305?à‡?ñ¨ò@O	V"À;Q4‡Ç	>À<ÔLR¾éµ@ÞÑrMû6@'¾´V?Áø­æ­ž‰¿«þym)N-?ê…¸Qì@	?Òñô¿ïãåÌÞÀ?ïÛ_W5¿é¦n£¿é~T>p©
¿bÜ­>‰u¿à¿Ýƒ(iAGNbllB3 1055+433?ïі}&é›?zbQSÅ ?@éßvÊ??
ÃÍ6F ?uLQZ?y¥×Žžs0?ïä×K'
ë?iNå_M"õ?5îJ•Eú­?AàžP±Ã?hjêØ-?fiÿ:ñ¸&?ïKUwfúò?ŒFåE(N	?ko1
Ãä*?v<RÝt?"'jì̶@?‰ÊþÍm4 ?ïöuP;?8ßÓBvõu?(°1'Ú?UDhhôn?P»Ýá³?6ó,ʾîÌ?ïÁم(.®?~öd0»8˜?Q¸ÝÈ\ú?Qª«·î·5?z¥5÷6A€?}9Ø/ؽø?ïª5ÝÿÇm?ƒo}-«žz?I6¿©Ö'?Xhöà°Ó?ƒßŒ#ù}?'¸L»Ü?îÐ0ë–w·?"9ɔ!ú@?w	O"ÿµ9?€·(ÓåA!? ÇT‹c?'vòN`?ïßUI¢O:?ZÒöyêÀ?C¹:{9±?@óËF	¦Ì?k¼h·\s?X]卾½AGN4FGL J1058.4+0133?ïqãùD@JbëÝ3L^À7æR¯Ð=À;0;pïVe@À'D@…›"/Õ±?"rºÝŒ¾?¨¥ã»@'»=XP#@ÄaՈ¿ ªÆ©¿áw¾þX
¿ä'Þ^ð{S¿ã³'i#°¿åc(X䝤¿ç&ÆsxAGNBLL3FGL J1058.5+01334C +01.28?ïï@ÒO?Rºåµ2Õ?>eŠ–~'?6üÈÕQÄ®?YøÂe•?OŽk%…{ ?ï¢ân'X'?ƒhÓNTJ}?\"T2¡±?bšÉYw­ó?ƒÅÑúÁÏ.?'þïü??ï›Úͧ¤Z?‡Ïtñc?sÿ<—¨+A?<"öR?~\"…§'?$xÜêå?ïÒÈÕzÛ?Yu"i*{?V֘-ØÞ?>Ö¯@¡8%?q¿Ø"{?V$¥kª?ïàû©•Kg?b)»:«.?;IÌ?gü?2AD3§s?k'­p«Ù¡?aGÓÇq|ó?ï^©b?œº£7}?o=õ¯XÃ?yêú%õ®Ö?™t'&îþ¼?š¹àÏÚ?ï™aûcc?‰›	¦ßâ°?sÜ®H}ŸI?€ìÑÍ?rÃ2A‹.?'','_?ïB&|QÆ?t¶*qŠ?h¶g&¼)?ZÿPÇ™<?'Ü¤á?X?qq‰KÂòìAGN4FGL J1058.5+8115¿å.7ö¼_@A_ d#–À9ÃÁ>#Q>À<¸Îé@'<ýâC'@÷¯~Þ,q?º °å¹±?Á¤Ÿ\&G?øQGñ0Yd@CäýÆö¿Þp*
ag¿æ5deÛ&¿æ€\a)惿äJ¯@ŸØM¿èæt¾˜×}¿ïóÓl#>ÉAGNfsrq3FGL J1058.4+8112S5 1053+81?ïí#-_?QSŒ}}€?BzÏxjè?7ÅíÂBÆ8?\ªºòx?NfgÑÉá;?ïáù2"¶?mOG"¥n?@ê¿´¢Ï?K†ì6Ø*å?iÌú5Á{?hB'h ?ï´Ó")VÕ?twã¶#5?]x,Ñ3'¹?bòN]ж?~8++Yƒ?q<2,ÅRQ?ïӉ™¾¤ã?UF¨¥$õ?NØM÷cê?/¹m~*?r`0…n•e?T_\m>?ïך1¼]?dX¬² Ý?YRç˜|üg?RÂÏæº6+?l:ò+@t‰?`k›Ðoµ?ï¤ú	_¾ñ?':çÈ~Æô?PK'¢t?ZžµÌ ô?"¸4À±H?€À&G#Â?ï~%Íøy?€WúêÈ¿?h…O—Y®?iµÿ/½^M?ŠU8Ÿ6o0?{Ö°8'?ït{±[z?x1'ä3aO?j"S1Ã?T¢g#rÇX?Œ^5‹U(?vV¶¼mAGN4FGL J1058.6+2817¿ë}ú"†4b@PCƒQX¸(À:%W¨]'À<vÄÀ§%@É{'G•Á@˜>{?´©8ÈôP?£×¡çñÁN?í²"\KZq@X¡C§¿ä|)±ª1—¿×ºÈ"W¿ä±õ桊)¿åñìa<°à¿â3͌æ-¿ä¥\{¬AGNbllGB6 J1058+2817?ï©­|ÞÅ?²Í™H¸kò?Rëyf"1?"Œ½õÒ1?ƒ7OÁÄ?°²ê­]q?ïá+àÈF?o/ú!K¯??fð¸¬l?JñQv«)?jç@óˆ?kVX›/m?ﹿ8†ü€?rc,ȧx{?XÇ‰w¨¥?^Ö`JÅÂ?|ÿñàS!›?p†-üqö?ïãm3ùÆo?Ji#‡ <?Kÿ÷ƒ]r?-òeh¼k+?e²Ì_ïL?GÅÊsú?ïÁÐÇzŸÑ?žŠ#YoŠ?K;¦}7x9?mt€À7È®?{°'t
œ?šàí<²M?ï *››7»?"xE?Q¢\°ŠïÙ?[ø‰ŒÛÃÿ?…Á
{é…j?'ÈÜ	!-?ï~,½g?€«a
?aA
®ï¸?`èÓsœ
I?Œ0[—á?}üÉá«A:?ï°¯¯mÊ?iñ»
n'Ú?bûÄæà-'?Ll;áxó?~*UB—t9?g8ÊЉ÷æAGN4FGL J1058.6-8003¿ìßµ~ÜnÀ2IêþæûLÀ8Òfàß©HÀ;ËûSÈÕ@<'UÓF@ö@×`¥?§Ã¾s?ÂÆ'De
@0¢_:ù@½r,mFT?áÀ½šTÕ¿Ðâî![Dt¿â֓ n¿ä‡âT1¿é|õSԓk¿ìð"rϏAGNbll3FGL J1058.5-8003PKS 1057-79?ïÒØz*£?eÔöK}*C?`ŒmÎ+?YYu ?l›E®Ld?^.A?¾‰?ïâ´)µ'Œ?rtïxò?;ʯ—h"®?L\g¸!?iҀrۄ–?qOð•kB?îGÚø½7?ŸEgŠ #ï?ÑÞ±0!!?—d°ìŒÿ¯?™2Â:›´?"⬹Û#?ïËD
9é?\#'ªß¶?Q»nÇù?>&ZZ ?uï4?œ·?XCIL˜h¦?ï}G}åU|?'Qâ[¯‡?xü0£pó?t‹£òkøa?"0Bé?y1é6XåF?ï´ò¾¬0?ˆÐ°iç:¼?\¸ º‡?x§Óÿ&'e?~_2™ž	à?…æ7Ù?íè›pšƒ
?¢a˜
?¢M¿ë+ÌP?›î&Dæ¤?žQX&?"#싇qÊ?ïq]?ÌÐ?zßi²>e?gÔôÑà?UçÂÈÅ1Ê?ázÅIö?xF¹.ËbAGN4FGL J1058.6+5627?×!{»7N @K7Y‰ßsÀ8+È5ŽWFÀ;‹ïXèÏb@B_ úa?ý¹"vD)û?šÀÜÿtê¹?§t®R¹5k@IÄ|œ2Ñ@§'ˆÛu¿Ð'¾^"¿Ür´þNúå¿ÝظG¿Ý…bÀi'¿âPÝèþÝ¿ÚbNAGNBLL3FGL J1058.6+5627TXS 1055+567?ïów;ÔJ"?F|ÎgøX¿?Ÿ…~þ?$»ÌÛ¬?W€áV5†?E÷iÓã'f?ïÌw?&±p?sA-åõ÷k?I0Âñ¸k]?O£ÈX?vžH#‰Ø?q¾À3{n?ï³Þ|«)í?ya®d¹È?[7n•´?kÐ(Æû?BÝ´Ì\?tÃ#ôn®?ïádáxwØ?Rçsw2å?@ a4â?%ì³,æ?j™VqˆÔ?QË.­‹•ª?ïåIø¹?_¥†ÑܧC?#N²àý?	Ñë
3"?iKÖ¢Îsƒ?_-4bn;?ïdolä»?sü|ô?`Þ #in0?hA"ÑZ?'V>dºuÏ?ŽGS.Xáv?ï ¥Dºv?'Ò¯"¥ñ?]B¼ç}?h!Fãõvz?"4¦•Hƒª?€ª‡oÎْ?ïÇ{ýÚê?h|lË0'?L-ºG¨ó?<p:*s#?xö¡Ϥ?gjÚw+ñÑAGN4FGL J1059.2-1134?ï1ϚÔÏr@EWçl‹C–À8*obŽj'À;ˆÅFƍî@0¿¿s@´ó\ƒŽ•?–Ä|=µ'?§*ò®~@
 "S.{>@#ùñÉ¿ÅžÚK:ö¿àˆbÚÀ«V¿âd["{L§¿á!Ä«–`¿å°pÀÝU[¿å7i=±;wAGNbll3FGL J1059.2-1133PKS B1056-113?ïóu©¶ƒp?C>H+vº§?"éÜZ
?Y–†?V·pÁŸwH?BRóN<êò?ﶂ;X5?{¥þAçéw?RkWþñ?Y?`ûÞ×=?€¸õX ?y!Š†,²—?ï¹Â±•ä®?xF]¥?YѶ—•?d;bš ›?|ªa廗®?v<Ø'?ïØd3õê—?Vð»ñ°-?Qc;ëfáy?8x×S7o?nê-à'èe?Süµ&vº?ïæþž£f?Y¼À€ZM¿?&6‰˜Þ=?	^ÿŸ§?gø÷Á£¿?Y
\efy?ï5eàÚv?•SCpƒ{?e,™œaàœ?pÃ#´BÅÖ?–º 	Ñ3;?"1[X'?ï¡¡½OŠ?'t&™ÏûÓ?^6ÿwÿ÷?i_Œø_nn?ƒÐùS|͆?6<è›ç?ﵚ@³yj?m¨'¿‡E?` ¿;âRÊ?Oϸ†ÿ ?}"€
aåÇ?jLï6ÏAGN4FGL J1059.5+2057?녗¨N@Oâ»ìª¸¦À:"'Gm|ÛÀ<o¼Õ±@‡Ñðøü@-›ymª(?Â;Ñ&ù"?®h˜Å´)¾?äsmµæz@	œ²êx"K¿ßÏÙ\'HC¿åF,iëV%¿å´üÌnÙ¿ä'zޢ߿ï\tÜJï?æusê³g¡AGNfsrq3FGL J1059.9+2056MG2 J105938+2057?ï,ÜóǞ¡?ÁÉF"¹á?p—nôbéˆ?—štâî?–>…ÅÓéŠ?¾=†Ã?ïÔ(){	È?vÕvf$&o?G¹ë3Ã8"?TQ«iˆÙP?rô­ý®àá?s¹ƒlu?ï°i"Žà?r‰c՚?`¶Q‹8ú?cvÿ[*v3?¢¢s\??m™€ÇÌ?ïÕ£t}š#?T ]Ì?X§æ»Ä½c?AKÿóP?n˜,Ò?O"‹ÂEí?ï‹iËJÁš?°˜êlŽ×E?^./FÀ2?{æþ՝%Ì?‰_˱]Ÿ\?®	GÚè¡ó?ïlY'ZŸ£?'Â""!RÚ?[…/j«äX?jœžYcrè?¼zäža?'™Qžxé…?ïb×ÌÁJt?'ý';î@?i$¦ÆyF?gaûîYª?€q—mQ?€ÐÕü''"?ïsžþ]h'?v­XªDne?s•Þšp×H?c†jˆwê?‰MQ,ór?qqQ¾D	AGN4FGL J1100.3+4020?ïàØˑA@OÈ<hfÀ:7|ˆçš®À<i÷_GŽ@ géAørî?û…tH§8¿?¾ÏtòÆ0¦?¼ìæÞýÝ@øSÜ &ç@I¾ð–*¤?ïsy³J¿âëÈæà>½à ¿(¿ÕJí#¯\¤¿ÙXI"ç«¿å#傦8AGNbll3FGL J1100.5+4020RX J1100.3+4019?ïá{Z"K&?Z{"j?—Ð?Cd<ÜÿpË?2ÖDíñÍV?i«–:¤I¬?Wá6ËA%?ï³åž›?|;µù?YòÂÖ¯ô­?_ÕW'½w9?€Zt:ó?w§Æ[+8U?ïèm<C}?r춊Ëô?a.žY`L?X=Ïމ•?‹:=¡è?qkm'ð?îžã$Òó-?{³—ï2?‡}@©…£W?fÛªû1µ=? 2}Š'2_?xypp§?ïÃuR3öÊ?p"qåÈ?Wï0vص÷?PGsÕû?xIŠÈNm‹?kç¤X«8?ï$!óÎL?˜@õ"2X8?q&Û/"ÙÉ?w"¡ÇãFr?—2
¸A"Ã?•r^ü–'I?î÷FRA7Ð?‡¢'e};?pa'ú?jY%¶Ìóø?œþÑpN?…,zåß?ìe?bºW?—»UiÆ?›°8ߝôm?"–ÙŸ
äÕ?µéù"¼¯?"ÿ*>®@ºAGN4FGL J1101.3+7017¿íñÖØ¥"E@Fÿ¼ä!À:CÃz=³ÀÀ:ìL>œóÁ@ÁÿiW@6
éh?·©׉>¿»iˆúe@G£áñø@]˜oVпÓÈ^˽X¿èéQgÑ q¿è]Áa^¿©¿é"'Ž¿á;Tiä ¿â\‹áõþÊAGNbcuGB6 J1102+7019?î¹rx *Ë?£"ª™î"?dšeÍõ?d4äÐ-G?£2/´ó?£73¥¢P?î«Þ­Acš?«†x™]£c?J'QO?beªó–ã?›…Ë­;? ®'¯E?é<tÂl$?±]Y"»? €¤òs+?˜I¡ªLSÇ?Æîð
Ð¥?¯cu;ހé?äûÜúíF•?·'h	ðø?q"î9"U?gWë"-2	?ÕÁöQwä5?·j'oèbƒ?•œVZ?§ı¶¡?tÙ`s#3o?u':;)Ù?¢Ùúš«áq?¦–«ªG¥?ìÓÅ~=·_?½^?÷øÛ°? ¦ë½!«?±¼	fHBì?±^€›.?°ûátÒú^?è'§Ǥ?°P
ïZ0ò? d¨½w:?•¸í'þO:?É¢"2¢>¯?¯
ÖGîØÆ?ÒâKtG¥†?»›0G›u?‡xæïÙY]?…Y>nÎà?æ0öª8D·?»Àå@"£CMIXED4FGL J1101.4+4108¿×"ð§`ö@O¹É>¢ÒþÀ:{V'Ý¶À<~CyÒSõ@ ·~"Z•x?ú#¶¾mŽ?ÂÅ Æt+?ÁȚx'·"@´ªFJ@‡¶HüÉ¿ð?ïÿþˆ0»Š¿Õ'îdw"÷¿Öh…ºêw-¿áÇq^-O¿ÌɄƒ\ì?AGNbll3FGL J1101.5+4106RX J1101.3+4108?利†kÈ?…K¹Ð?NüÿŸÊÓ?I$Œ*fG?"(ÎdÙFÎ?"ñäçÔBÀ?ïË:ßä?x+ɏk?R0—I°^?[àš%WíÆ?uê<³àMÐ?rÛtñö¨@?ïD¬SâÒ?˜>0ÚkÛ?nýLî,…O?{ÞW,ma?"ŠËþú$'?Œm Üå®?ï	Hå2Z?röŒ/îñ?Eɀčò?^m«$Ÿh?—pøÓ W?p\¡ãŠi~?ï¦ÏÓp­?…Ÿæ6k§?_[ޝ6¶?TEÏË5o7?'`a-S¸?"¿ýÒp†?ïgº#|ÜÊ?ŽåuÜp?du3˜9Æk?lp]Y¦%J?zûâ?ŠVœ{a¥?îÚ°ûŠûF?'e"H:Æ?pmóbۃ?x¡3Ï4å÷? G1⎯?'¼"¹Ÿ…?íÍõŸåõ#?ŒðÉ5¦p'?BA•x?sq¢ñ…?«Ð»)ìu?‹1oës¡¥AGN4FGL J1101.5+3904¿èWñWŠoI@P
j½ãû½À:ÊbhÀ;ÛHHn-Û@å	Yšü@·Káâ8?½š)¡äì©¿£âX¥2©ö?ä¤d~.Ú@¹ññIƒØ?ïþ;â¿ë-i$†È¿çWöÌz—v¿åé<oŽ¿ïþ%–c.¿âïÃÙßAGNbcuCRATES J110130+390434?ï'wEÔ?¬
)æÜ­?wðÉÙä?˜n|Tå5?€6$rë? h-,\J?ïlíˆÑl¼?k>H‡{?q…®e?Æ?{Ò àÎ]?ŒÆ|ò1?†Œ\<"p?íýã´V£?œ'}šµ?"˜ÈÓçj?6ä¶gI?¦U`S®§?"§ëÍá"Y?îá?'nQ9?:3œé!?ˆ
ŸãE"?rT—´¢–'?—ÒÀ4k ?xÒÛ·"Ïä?ï€áÍ÷?°֊sˆy?"ÑxÞf'?®vôév{²?…=ˆ?ˆ3Ì`@\'?î"ͨâ?¥#÷Ÿi?€ýÈLEb?ˆˆqC³4Ö?¢ŒQGöX?¡Š €®/6?ë(°3 '?«ç*Ÿz?¬¨ñ×Aqš?¡žš–ae?¹"A'TR~?¡v@®XÞâ?ìCÑpAþÊ?¡~Úú­Â?§¥'¿˜ƒ?š²w""ª¥?²ð4þ0ê?™›WRÚëAGN4FGL J1102.0-6054?áYz)^?ž¿éæúàÜNJÀ7äè¼í[¹À:!_Ìqç@ñèÒ@Èÿ΁Ù?¶Hê¿üÚ²?Ñ XšËÈÁ@)Á¡ŸØ?ø_Y	¸&?écáPè¿Å§¼Ýk€'¿æ|fÃÊÆ¿ê"eҐ[¿êZ³R¨D¿ÕcŠAGNbcu3FGL J1101.9-60532MASS J11015838-6056516?˜3}ƒ'V?ÙµN½?çï²@=.?ÉO\Dà•é?Í:ÓP¦^?È_PWuï?'ÔÑÍxì?•'³C¶O?âDŒyre?«·D`"O?ÚI'¾W`†?ÂÐ^ÊB?°o–ÓÑ? h"­»Sl?Öftá~`?´ÕÊ—=?âɔWª$Æ?µ	BüBË?w•älGo4?ZÓhª[Ü;?݅òM9ï?©KˆD«­M?á
Û÷
?©->T3ô?"}s½Ö?€õ0pA¥Í?é=áùjöª?Ä~Y"Z&?ÉƐCjÊ
?Ä'j³?z[ø©J˜?ƒFqÍÑpR?ä¥ñÊ;?ÇÉúµhW,?×db87°?ǚ8âþ~?£Äðê¡9š?—éU—×»?ÙSQê6?¹E3E³"?â:H|N8?¹4S™°Û?PASJ`´¶?;¾ãemÍÆ?áÍ›SØð?±ä™±½2î?Ü´#vZWî?±ÝڒèbpMIXED4FGL J1102.1+2249¿ïø»ºD£¸@P;$_ZÙjÀ:Ö0ã͚RÀ<y,;È-+@øãýëÓ£@
…É=?Ñ:~¯"®?Ïg	y{l?ýæª|¦D@B9_E0¿•CÐå5Nk¿åg©\…<¿ç›Ò>%Õ}¿ï=ò@¿ïՀ/eHY¿Ó0æ"ÀAGNfsrqCLASS J1102+2241?ïW뛼V?¡TSk×?m4¡všÆ?où%›õ?š.nW•uð?Ÿ"ÇYÁ?î;Җ»Bâ?«~â=Îø?—IkÅ%,˜?¢¹m÷Èl? ž ³q	—?™"'MâåR?í€{£9€? ÇÏ\?"‡¼5͛?ü{0—?®4g{9\B?ì|=ÞÊá?™ç?‡9l³ø?›Ÿªb'0?€?þmÂ¯? ·@NÉ‰?}kLvE—'?ì¿ø¡o"{?½¯f/V?€;ðÓ!Þ?|ØÅØג?·øÚu®/?¼çÖ±…§'?ëBn&E±\?½JG<ª€?¬½Ojò\?³ŠöÛÂs?·çÇYî?²ÜTòN?ëR˜'S?§|צvu?¢%šhë'?—'€~<1d?º'ž7Z£?¢û¨‰?êH¶Ó™Î%?¤×øÚ.М?±·F`$?ž#­q_5?¼"]·?ŸõF‰>g AGN4FGL J1102.6+5251¿îâˉ"J@L¦&€IRÀ:҈
%ðÀ<ʵ1¥"@V7éPf@¹eç»?˜ùJ"2ª?Ë*Pv%ã?úI·¿Ža@xh??ߺé
55¿âÿ^šj¿ê˜±¨ó¿æ>mhc¿ïÿØȃ'ð¿éd}Ãz=´AGNfsrq3FGL J1103.3+5239GB6 J1102+5249?ïHÙÑÔ.Ò?½µÌ.†?‰.r•Z
?±ß–춺?"›ëKw?¨5PÉåõd?ïÕ߁Êç?r	ÖÌá?J7M?U¥¡]‡îj?qÉ^¶M¹?lƒ+ÚrZ?ï`ü,"f2?ˆ¸ãЎ<2?s‰À@sùÒ?x/*¨Ƈ?ü²p½?…-,<ud?ïì|sª,ö?AÛéõfâ7?P4»K?3¯
qN÷?V…äæàþj?:;øhÒµ?ïB̛y˜?ªÃ¨MøÅ?"9Gµ¦^‡?—Ùüò?´1?‹'tŠ€? ^`Q‡.?ï~³ïR«?Œñ"tšn?Xßuν­•?e°³b'È]?7d?‰Ü™3ó@?î·/uÓ/¬?•Vþ2ƒ1?€ÛÓ<]í\?€úîód"? VÔeuå?"‡ïî§ø^?ïÂ;'.©G?d¨3GЃ!?gÜËYo†ð?UiÊH·?rôÍ!¤÷?]åýæÄFvAGN4FGL J1102.8-0148?Û~4R0é@I~þ£ßm¹À;¼pñÚ£OÀ<ÏQÕQ×@#E@tI	?÷c¬bäÒ?×(§¾öJu?Ì<ì™.:?õâíÖ1Ð]@J}ғ¶¿ïÿ^à54j¿ï'7*8¸®?ïøÞ6A?ÌõýR.Ì¿Ðó~}ÖÅ¿ã8ì£^iAGNbcuRX J1102.8-0148?ïÎ	J#7?lÄlÈ×}?Ge'´€®D?8æ!ÚÉ?v¨'mnÛ?k(Žðr
?ï®Ì]Þyë?ˆˆ¢¤¥ÔJ?TÆx>'öa?a½úJ¬)?´r ê•?†HɔÖ]½?îÝÂ迾ê?ë³-C£ü?a/Q7éC?_ãLrù·†?¡Üa¹Z4?Î4v—Eˆ?ï›Ï¿E?€›¹0ò?I §}»?:' ›c«U?›Ä+…Ã7ž?€~=íQIÅ?d€:Ö?"qÛiZ?T»*Ü·W?Kø—wÁÖ?Š…Á‡WŒ?ƒy$¼Êa"?ï8°u´?ši5b]N?b¦,;%§¦?pÞ7:wGÒ?–•+ÐÝ5w?—ÿº1€ç?íÿb^ñ?š:õ3<T?eX™1/q?huqՆ?®¹d•Iár?™ôҎþl?íN=ò÷%?Ÿ	Çt¶DÒ?VÓè"0'¬?VÖt	úY?³š>n]}J?žèØqÊ\AGN4FGL J1102.9-5628?ètÐ*¿
0@
J¡¼}Ê0À:p.Ï÷#¸À<¨(÷@ »a•qA@:ëÄØí?Ç8§?¸Ÿ.ê#?íè*Át©ö?ÿ?®3Yž­?ïÿ!Í°"¿ìTç4¿³[H¿Ñ*™¿á‹	³Ýè~¿á%&_楿æÔù è­ÔAGNbcuAT20G J110315-562635?ë02/R(?²rP´HRœ?f¸–`\g±?Z."ύï?ÂäTé;mi?²]iÝ¿8e?ç^õäü¢?ÀÞÓ>Ï?†=Öcõ(ÿ?†\]4IÄÖ?А%ƒŽ?¿j/QYíe?ìd©S0÷? )RWl¥?€¡O?^1à?sþgô5ên?ºÆíjÉ?Ÿ]6òz"?ìƒV˂Žª?ŒÒJ./9ë?"}ºÎšÉ?dˆF?¹U'HÎm9?‹Ä±ºh+?äŠûŠê&?Á6éᅖ'?xóΛ½a?làÒ
$?։¡N?Á8ߥA˜|?ޅ"˜Âä?ÇY€Â梔?Š_ۉˆg^?"¹ïòÛ7?àS¶EZa?Ç<Õ¤Ÿ?ç¦*¾}—?¬e®™P¶‹?1%:AÝU?~dŒü»'?ϔB³"þ?«û27v!?ç‹yEf;ž?¡†Ôssæ?"—'{#tÀ?€Ò¿Á¨­?Ï?5ú&»ð? ÃxÈ
<¼MIXED4FGL J1102.9+3014¿ÝõÓ4<j@P"
ú/§À:¢.›
³À<"îNý"@YÚ;JXê@!ï#8ê,?Äܸ¨'¦ã?ÀÖYh|?óQ+¡nz1@o%ý•—¿ÑW6]48—¿ê€O ý7¿é$¦©L•¿ìYƒßž
¿ï̚!ÿ¯"?âÉËûìu	AGNfsrqB2 1100+30B?ï»bº'ì	?€§ÍóîÉ?xU©¶
~4?~gʧtÝ?cñò'zš\?`–(šŽÆ?îÚi#ôÀ¡?¥¼
-'™×?ŠH4Óðx;?›BÍþý«Ð?—ŽÁNçÈ?"ØÑ	i؃?ï$ÀÝ2ÿ?†$9¿@&Ÿ?wõ;J•º¼?u5†±à'?•j•‰º_?ƒ ¹Ç\?ïmÕ*ŒF?tŸ?¹Q»?ƒÇˆê½ß?ohغvrö?€Ã5¾5¬Ë?bl03ˆEo?ïMmR'˜?™oݬš²†?'v(Ãq?˜_h±ŸhÉ?sp³Æ:gR?rm.vžäz?í#»oh~Ö?¶'I
ýÿ?›ÆM6&ž?§,:û<?¯á"o@ª•?­þ4'=ËV?îUX½d»?'á@Û_'?ƒú=3jM??}Ô 7æÉÀ?¥«äÛ…†?RÒȪÍJ?íÞ
ØÁß?5å«p%?£ßâª'b?—aåâÝ?ŸÍJmb?‰ÎýÙ©úAGN4FGL J1103.0+1157?îtÀ	¬t@N6#=òªÀ8ø€'Š×_À<uƒ9ÛÄ@ÌwȹlÉ@aGãÄ`?©6æ'xÀ?¸ÿXÿåAÒ@
@-¹€@çÀI‡¿Ø9ã{î¿á¾«6z'¿æt~¢Gh¿æfOõá™
¿ë aÉÁ¿Ý™åóíAGNfsrq3FGL J1103.1+1155TXS 1100+122?ïèWî1) ?Xр™K¾?E•@Y+l?:̀gì'Ù?bBÁÃqÀË?USFŽ'$?ïØJ½F$°?o{ÕÍø'?Dƒ¡,	Kø?Qï­®k¼%?qJ-ñr8?j±…u¬ž¿?ïipñÒI?Œ>X]í¤'?qnÎUí)/?x"?)bX?Œì\Møu6?‰'ƒI˜o?ïü+ ]?#3ÓEÿ"þ?¾qÖ
?1쥟?6·{¼ñÎ?´ãô•6«?ïËèz|ã?uvÂ.À?L‹a£—?A2َêF?vz'¥\+?to:"K<?ï'ÀyNÂÓ?ˆ#žÇ%½?[¯œ,÷Oò?t"V=2=?ˆî1¯!,?"ëq¦×ò?î­p
'm?œÖ$4HÏ*?wÓ{ªÈ¤?xrGßd_?¢.}£?›3þíØÌe?ïö¹|&ÛÑ?A£_ë7^f?2Û@çt»°?%Níÿ¬•?K¬n!"VÄ?=ÿÛ%:hÃAGN4FGL J1103.6-2329¿ïÀ¶Íö²=@@‰ß¹8›RÀ9ï(ÝnۀÀ<![Ao6@ ø/']5?üNÞõÄ<Û?µ/Gì'Ü¿a*8'æÔ?«àÌVn@Y­í¹?íÕ»=®6_¿áâû{8†¿ãÌ?Ü¿Çïϛ´&
¿áÓìCÇ«?c…—ÓPAGNbll3FGL J1103.5-23291ES 1101-232?ﲨ¨ø~¤?ÙõÎÿz?Oæ
d'Tõ?F"]Ào?WtïŠÎ»?€æñ¨Ü¨?ïÉê£ç;?vqç°÷,?JL/Ÿ,ñ?QN—ù›?wÊDj¾¾Û?s@QS¥?ï'U?³°W?Š™š9_o?cà®RL¡Ä?_ÞOÍcóµ?˜™B>tÝ?‰O¸ARð8?îÃMâà?{î.;e¨o?q•~nPXÉ?RÊ·" =?¡››fL^?z©­lðþ4?ï~R<§"ô?ˆd»+ê³?^ŽïI¶ñ±?U;›Oë¾?Œ™'ýbÇ?†]m?g?ïmæ¼åŠ?	:k¹?Y–l̅¡ä?cH*Ô{€?©Õs[ä¥?Šð_0䏼?îCˆÓ£«–?–D=ǧ?s=qJ|V?n?I¢N‰§?©_ęt5?•JpK3?ì"/½1ú#?˜Œ¹S¡§U?ˆ"ç¶7N?q›\üR?¸Ìaš?—uÝuéžAGN4FGL J1103.9-5357¿œhüŸ¡'"@š½†ìÀ83á
Ìq]À;Tª:э&@‰K+L‰ñ@-ÑyÚ·q?¢ß#í"¶?»p´yß@kK¯Ri@2("ž¿Ù"iʀA¿Õyœ^E¿ájè¬&d¿ám¬@eJÝ¿æœÜ¤Zé¿ê*ȀŒØ@AGNbll3FGL J1103.9-5357PKS 1101-536?ï™×–÷ ,?"Ï3€÷;?S`©ûFöÊ?Tk»e ["?‡÷j?'Ñ1¶[q@?ï?6&¶*Ò?žÒ¤ä6±ÿ?P¼Œ¯n¢?^֋ç¦)6?—?_¿ÂÉ?ž'*tÂJ?ï\!áH§?"»¨å?}> I?ƒMá_­ñà?•í,IÒ4?'IºÊpðç?ïÇBF¡z?_&˜]=ú‹?D•2PÆ?/@­"þ?yÌ8è%Ü?],äó,Y?ï[ˆÖ—•¢?ƒ´
C.5?Oì
§;‰þ?DžË©"ß?""¿XJ8?ƒ\à†3$‹?îJN¦½TÆ?±þ‡î—
?f#üp?wz¹#¶Š3?©ùóV¼^Ç?±°°V3K?îçêÇ«ó?–ß´5E>ö?~ýÅ8U?ƒß2éŒÚ?›C5¿"Ê?"Ǝৠö?ïtd¿®gm?z{IÅlkn?Y:Ú§ ?IùŒ­Ju?¿tÛ°P¦?xöjt¤×åAGN4FGL J1104.0+2611¿»B®æ²Ñú@PØ¾r–öÀ;-C8dÀ<Ì]°µ?@ ԁ÷çX?ý?óÖ&ã?Ò+ݾâ~e?Á,á	š³u?ïUa%´Åo@Æ̝|þ¿ä9&A³¿ïæ,Ÿ›;Z?ì°Âtºg¿Ñ´îV,\¿ì^ܙÉjB?É/-5A*AGNbcuSDSS J110357.29+261119.1?ï	ÉSØ?‰ÈfÓÍÓ?bµµ®$?`q_\¯?‹¹ÑD4"?†ß­V
H€?ï¥@׌?‡ô˜¡T¬ˆ?_5íaÉõ?r›ÌïóEš?'ÉIôƒÓ?€ý±¶ÒØ?î߯iº"?'h	ëwn?v­m%9÷?xí:ܙüD?žqîÆ!?¾PiA:?ïR›¢4??u·¾J6…§?joV'¶Ø?_uù߆	-?'^¡ƒÅ]G?rŒŽMF?îá³aŸ_à?¤@B
·?ss	Õa ?md_²?žìÑT9öÃ?›¬ORh¼?îì[ÿ?¢Þ‰uÃ?pÕ~±'²ë?}"¬H•"€?žHÔôÓ?ò?  ¤Î?í²Î9g?¢z溯tê?vÛÖ«ùè—?t'uýË?°ûÐÉÆ-?¡ñStî«?îm§Nt={?'­3ÑÔù‹?s'q¥Ì?pˆÿ1ÏÑ?¦³\ù«'6?'"}ÊëþAGN4FGL J1104.0+0020¿ïÈÛµ ®@JiÝS¨À:ÕÀOæÈÀ<CHɝm@³k;p|@X¥}Ójv?Çg}'Hs¿'Âþ†r?Êd|ZÞs@Ga¶Scª¿ç¥ Jù"–¿æš¡¬bŸ¿à:â‰Ís¼¿îc!ãT¤?Æ8'}sHL¿ïÒìk΅4AGNbllNVSS J110356+002238?ïÄi¼å¬ ?z4RMó?SÐOÌ»—?SP;œƒB?y­€Å¤ó?w,ääˆ?ï¡J—Ë/¶?ƒûö¨·Èo?[¶#ýÝÿ6?cmÜȍs?"6•"áLž?€š²}©®?îàÏ
>?ŽþÚ)ñZ?veTÔQÖ(?zgôù5é?žLɅ:Z?ŠÊÓæV®?ï°¯›õ¥š?h÷ւt	?6À~/voï?,\لjO?ƒÊ{¯?h\"]ª'ƒ?ïwÅì*W?ú¥õˆÝÔ?d<@ºÄ\?fúUíÚzì?Œÿtي)?Bª;Ö¯u?ï\µ¯ò?¤(ÌQ!¼°?frĐ	Å?uYxêy?œú÷s¿?£!ÐRpî³?휼äæ"?šJå 8ð?ˆ@9AoU?"OåԄHô?°¶œðÍ?–Ã["Â[?îä™K|ç?Šëv\Ýäh?To¨©ªÒ?S¥'"'?¡ò1F…1?ŠGZào$AGN4FGL J1104.4+0730?èî4Tà÷@Lùfb4¨~À9ÎÕxlù(À<RæP+'~@ת«dÈ,@ϋÃîú?±ˆŒÖ脎¿ŠÚ6ÓâÑØ?Ø.‹-Æè@ñÑØzU?J´·,Q—¢¿æT²^âc¿æWúȈšn¿àzó†tù§¿ã{Ö[åÚ¿è-ç>"
¹AGNbll3FGL J1104.3+0730MG1 J110424+0730?ïòÒĦ?I`è'Ûþ?2š/Žn
?!'©7å?V=Ð
Ü?FÌéo¨Ù?ïߍpZIç?mðµ¸Eş?@}B³Á¡?JpAG§@B?lS?D'?i ÷  ΂?ﻟð9¨1?tœ°ñÞ?RZg8Î?T¢§:é`?}¬ñGýÛé?sà'¡ê?ïê{K¥ÅÍ?DŒÛ²ôM?H÷cùbØ?,;l–úš?^åLõ¢ì?@dÖ団?ïã,,%DU?`ö³ïéÙä?A"oìX1B?1-™/¼<?hn÷êê½v?_™s
ŸÒ?ï"e.FÔ?¼Ò¤j<'?QÙӋLä?\§³(ü?ˆÆY+š"?Ž§RQÌõ?ý_Í×?{Nž•ú8?\†¢Pc{?Z˜Td÷ø?‰ìbƒÃ?y6®ŽX}Ý?ïÆGº D;?bâH<^¾?bMÞEdm?N·JÁ$ß<?sµ3ç*Ì}?\ËRoRºAGN4FGL J1104.4+3812¿ç%ÅЕjq@PBIёXÀ5•v¡G
À:Óyq@'=ŒþU±?ûÄ£ÿYè?z}xf»?"×BÇzÓ[@º'®š²ž@Ô9ùËÞe¿Å¦²Ü¶¤Â¿Õ$è[Ÿ¹¿Ü‹Ù?Áa¿Ö¼/ʱ•¿ÞÙTšŒ¿ÓH__Œ«AGNBLL3FGL J1104.4+3812Mkn 421?êØdtb—?À|%?Pܸ§wºä?[-)s¶Äï?Ŧäþc,?ÀnŠ'€?ï˜1»Ÿ‡?'ùh€)؂?ZA»«$Ÿ?p'HYc0??†«Y¼]3¥?Ü–Ú§ŸÏ?å¶L0Ò}?µ°ÏQr ?'
¸ù{ït?'ÉjX¯"?Ós
×a®Ï?´t¥÷fw…?ïÚgJo˜r?e
n>SM1?"Ê͓·¸?YºedJ‰?r6>îG?dÝ¿zµ
?æ9;›´"?È.ºè£¡?Pš-zÓ?Q!zU	?Ó|îœÅý?È+K}àë?îܶ8Ùä?¯žP§Q,?g€ÄPFÐ?z@DR
? ¼54É?®a‰lÈ"?ç"/™w?³Q{Uˆ^
?ŽðÕæ]	?')›Â¯5º?Ðþ̯º©?³.[tOE(?ïʚOntŸ?uãhpZô¬?''Ãm×5?%=u¬Ï¬s?yöÈ:Ã'¹?uÔ~'‹AGN4FGL J1104.9+5748¿è#ÉlßÁ
@K	pŸM8À;cpè hÀ<¿Pû›@Þs1s•@ÈPïܜ?ÃNwëC?NVq¬˜@	æ4á‰t¿í⯢št5?ïÚ==£#±¿í²•~æ¿Ò•!û'~¿ãÎCYñãÞ¿ïÿûÎBÓAGNbcu7C 1101+5808?ïöŒ0ÐWq?]´©k!û?4ëmۏÐ?A¦•ª"¶}?KY†‹8µô?V—nU¤öe?ïâxۈý??m°¸Ÿç7?;´‡ªæ?E ûùG?j&­¬‰ªö?iÂÑ@
òK?îÔ­ª®Ðõ?–Ɲ/f¥?r-Fv'Fª?|µ½Þ'²ù? o|…NÃc?•®¬©f¢?ïós=N?=ºd6Üã?Aéªf?á´?-e-	Œô2?P$°öeU?5ÿ©Vta?ï÷†Aݤ?W	çV.>'?;Å_¤>æ³?IdæÅC÷V?DÞ¢xÿ?Jš®v̱¬?³"|Q?Š°Ð48Ö[?Pûkb'Á?YŸ¼Ë?ˆŽÓºI3ó?‰|=ƒ½;?îkՊÞi?›x1q¢?v‡i½B?€ ¤‹C×?¦qľ¼E?š
:`?ïڕÿ‡<?^y»s›õ?^ÕÓ±˜hí?RÆHE¶dù?eÿÒӗ¯?SYC÷$[ùAGN4FGL J1105.8+3944?î¨Cïª-¢@P0O"}ŠÀ;/øìÀ<"Ž7£@N´¾c(@מà*w£?««u+%¿¶ï«^"[?ôÏ|ªuŠ@ƒ+ÍcJ¨?ïöaD=¿æ6M½øô¿è;$,/3¿ãÓø:8àò¿Á')™¿ç¥0 Y;ÛAGNbllGB6 J1105+3946?﷏ï\à?x"-æ…O?S™ÄȀ'¨?PM¾3ofL?Q—¡?vq{ tw?ï·~¾:Ò~?z"èÀ~E?V2óyŠ1©?aWœ»Ÿ?~³ãó(Ø?u2ÿ=Û«S?ï!•ÅŠÊZ?‹ÁyAj?cžfn/CÌ?fÀÀ–/ò)?™Yz‰wÒ8?‰òú'Ïä?ï¨H,tR?j"YÂcœ?XiU€NgÂ?Gª{-ðsc?'àÓ8Ò|‹?iGܺŒø†?ïlÒóú°'?Ž¨Žé.?cRÑyPï?Z]"5žcS?öŽ²Íז?ŒžÐGþÜ?ïDûqØ>?›Ø¬«¤pÿ?d«=ßø6?wP؇Ût?"ݼvLê=?—'äVqÊÊ?îTú/g!?–d'ÏÏ?jïYŒÒð?e(DVÃôs?©i%'Ã?•ÁÛÇÃL?\ÄH'?äa•¦'Ò?x!î¸À?pSØ,Aö?£´øŽh?ŒôڞKÎîAGN4FGL J1105.8-0731?ÚB6LS{ä@Gx ě¥ãÀ:ž'jöîßÀ<yÿ ^°@™½€Ô@ˆR]S?¿óâæ>¸Í?qbÿ»Ô°?³|{P®CJ?þ!/}F&Ö?ï¦rÅð9¹¿ä†ÿ=T<¿äûà^d¿Ù¦-¼%à¿áE}Ð:k¿èppçɨAGNbcuNVSS J110547-073235?ï¸z؎L	?sk¹è"¯¤?Tö"G&ª?B³‡Ð¶ƒ$?~…ëx¾?r~́Rò?ï°¶QòLI?x*ZÈ&¸?Sgßø¤G?S¶n*nØ??eo†Ð³?v/µMŸÞ?ï`ô¤N¡?}¹…ãz?eŒ±ß¢›®?X—´QÉ??'>k+ºFw?|uät
Œé?ï<pdü?nèì"p–g?{Èm¦¦dZ?X½íoZZ?'‹v†¾!n?i·±…Ëî?ï|3þÆUK?'eI7+èH?c§þfk҉?Sž=* m?Œ	§HÊ?5ý.~7?ï O•-h?ŠƒÄi[?fÜ¢T7?l}øbْN?™‹ë‡Ø9?ŽmqUT[§?îæãúÄ_t?‡a—^k?q6·aû?]CÞRŽsÈ?žÕÒãoÚ?†5¤¢mE?íÐñFv(s?ˆ;­öµãÙ?"³ó^Ip?v¯èµ;ƒµ?©ñç—?"À攽õkAGN4FGL J1106.0+2813¿ïÂ}ØÆ@P«hœ¡‹ÖÀ9TWuÇ,À<NÄ3¡<@ýñò¡Æ@®iŸÖÊ}?«ï°GÀç?²‰»ÀŠõ@¤m'ºZ@f,I	3Z?äQXí×ßP¿â	û+"é¿å±€`b–M¿åâ£cF÷5¿èۅ⭉¼¿æðÎ3Õ¢AGNfsrq3FGL J1105.9+2814MG2 J110606+2812?ïç`pqñÏ?x<¦=ZÃ4?<¹,ï
ʲ?/*{ nj?ej7;Á?x'Ñ;'ž<?ïÒ,&ñÓº?qýBÃlyl?GvìÊ@'?R O:qá?sûÐ¨F?ny—³÷Ñü?ïªÊ=¼¶?zˆ†TÆ?]ƒD¹‡'?fϵjq—)?ð1ÔU?wc"ã v?ïæ>v:øW?JM
=|Rƒ?Vÿ¦ˆ$Z2?>_aHå{y?\ƒl‹¸h8?BO#JÒä?ïμÕ͖:?rQx2‹¬h?Nóõ[X??|gÏQ?'?tÃ2¹Í€ü?qßî¥ØÖ?ï}y¤ wž?‹6…ûæ|?\¹
h£vu?l†‹¹øÚÖ?
u ~Õ½?ˆ…"͗ð?ïS¸«F"
?ˆåäÒ{X?lþ
Ä/5 ?qctG¸?'é(â$±?…Ã	Ó¬â?ï´p±²®Ø?k ¢˜_ù‹?qY]
ª&?^ƒãã¶fŽ?tnJ®n¿?b~Š±»6AGN4FGL J1106.2-1048¿¤á¤+9@F$ÐgŒTÀ:÷!' ÿTÀ<U1Š¼‡@ôðVÝØ@Cœzª?Â\x¦Ú'¿–¬fzÞB–?Ò»-½þR×@¦`s^™¿ïÒ͖ h?êÜøɪÙ]¿âyJ]d¿ç#•Þùö¿Ô±JG
¿æk¿Á¡u†AGNbcuPMN J1106-1048?ï´3"·æ?vs@eÓÍ?Qx•º%N??ôF+ˆ:3?€Ä)7ÎLÐ?uÜh¾µÓÑ?ïÕJ¬Â?q5ÊÀj­?Dutªí%°?Mkš_i«k?rËû^+†?m8†C¥k?ïXTóLhc?€ÌÄ J¼&?i&Ú=°[?cÑÉ,¢~ÿ?'ІPø§,?}wÌ5.?ï`a®_"?eóÝ]ïÄ{?c)ºMyŸ?MQxq(?‡]¡\5ÔÜ?e2ÞrÍr?ïoBÝ9m?'MYH÷bÉ?ce£ì+~]?S×5ˆ"g¾?Uß¾=©3?k1ö ò[?ï|Ô1Ej?‰ù1ª~
 ?T¿ß&?K?_îÏk(?Ž2÷כ™?ˆþÆ8?îÃÊ/8§¼?‹÷é["æ_?sý×¿÷"?m·M=^–?¡C¢-q:E?‰jZœ»L?îÎKhšYn?ƒ
£»ê#
?vY@­­Â?gW‹VÞ§¡? P'pîeà?'ƒfºé²KAGN4FGL J1106.5-3646¿âEn¼§@5€"xÐÌ6À9ÉÌIN†À<D¨£!ؘ@IV
M·@ƒŽ)ùΎ?´}íì'Ô?³íóŽ¶@VÆž@
ï6ŽÝS?ïÿÐß´¿Þg=;tË.¿äø~+	Ë¿ÒÞc£",¿êJÔø³¿Ô¬Âû<ÍAGNbll3FGL J1106.4-3643PMN J1106-3647?ïä¯Ü?ö)?YŸª¾B?AµYŠßñ
?5TDئ–?fâÍkãeÜ?V"Jð5?ïÉo²>?{¢=±6à?Vü.üÐ>?eÛðUæÚ÷?u‰i~QrA?rùücû8?ï†U1p÷?…u>"'ý+?mS®ÐÄ?xeÏbâL?‡$#Ä×ë!?~ÐR£=È?ïmûT¹Y—?ešZu˕á?w=[È®%1?U¤öžr;p?ˆâ|üم?a2ô€dN<?ïÌiîV¬?jÑB•_Õ?QÁ±EÉÂ
?Dl»'
ôÛ?uZœ'E?h/¾¶íé?ïiÚ—O?'c1â?i7Œó¾µ$?tÆZö¦O?;›ÙÝ"þ?Š+6®v?ï4"Šø'U?·ÔÐÎÐ?uÆïPÏã?|­Â¼Ä¿'?"û²Ï†ÌŸ?‡u/!Ä?îbc|HJ?"Ј½*!Ï?']=8hÓÞ?wÁpéó1?¡+)ŸAÁo?~7鶎aAGN4FGL J1107.0-4449?‰˜7ÍTe@,hÆ÷ µîÀ9!—q¡-À;ã¬ÍSŠ@kêÈ5cd@lŒPû?²
	È««?Ñnîàå@¦ýòÆ@D€t¯_¿ÌN
$=H¿ã•è41_ô¿éÙ(?º*3¿ë"` SÈ¿ëÂbæ%z¿ïÿ£NNA¬AGNfsrq3FGL J1107.4-4447PKS 1104-445?îæ:˜=Š5?®¡L]ª?žÕn–g‰G?®˜é`ûD?qŒùt^ðP?gï€y_®ç?ï\Z[7«Š?©•Û\Ó,È?xßÿ}¥Òu?˜Ì"›?Œyi{Ù:%?œQ·Ðã?ìªøQ4ûà?§`÷9Ð	?¯†]í:
j?¡Ë "2>?¥Ê	é?›xKËml¹?ïrOƒ "?nd6=X?ý?cX½ùw?bÎ

2">?ƒºrÖVüK?büéþ<ƒ?íÍYo]?©§Ñ÷¡:7?­@9ˆ9?¨"IB—"Ö?‡¨¿º06*?r0ȗ'?îdqs(ä?±'KÂK>˜??@Ö¶Ü?¥ÏCý3[?¢isÍÊ?¦$èü/]?ëb)ex2?¬ø5˜S£Š?µ`Ûwøn˜?¦–bn¿cH?¯¸»om¦? Ncç
Y®?î1I³14?x˜Ã÷á?›±êÌ÷"?…JôaŸ?ž$ߗÜ~f?'œ»ý¼—ÂAGN4FGL J1107.6+0222¿Þ? î'\@KvX£/D'À9ÙÒø_øŽÀ<?x½€ÿo@¹Ggž@À¥ýU*Õ?´ÀÿÚÁ,¿Œ:Úzm?ØuzÖµ?ü]JÑ_ƒž?ï••9¹¿â$çî'C¿ä90m†X¿ÚÃ*¢8¿ÚA	8x¿ç0ãݵ}PAGNbll3FGL J1107.5+0223NVSS J110735+022225?<ùýÕ?v¹š^œ2È?_w)U"ƒí?KŠX:ˆ×§?‰ê‹˜‡ÈL?uw'Vàÿ?ï• Uµê?ƒbl/ç×?anß)CaÔ?f†5JüÞÑ?†\2¹nSÎ?€:~åñÊ?ï,(¯nž?…ÁÓj7æ¨?t"Ûë2ô`?s$-"?•U³ »&?ƒº˜lq?îR_"¶š?'άpÂÒü?'	AÔ(Q?q<¦¬´J?¢Um1+7?}S´®Ûµ?îïÓ֒"Ž?‹6⌟°?t
r0Ø?ež¶0́?Ã(Ç?ˆà5ƒqCw?îǁKšS?š•"³2è?vžRðΘÚ?}¨HÖR? ´ ìOB4?–üܱ‡§?îwôÄɯG?'Èþ™Ë#?€ò¨a-h?|ý†+:YÛ?¤D	—žæ·?PÖ¡°ì?ëŒ÷KjPp?› Ù,k=È?§1îÛ,›p?ŽÂKiŠÞ?·ÿN6;GÌ?•¸)׳¾[AGN4FGL J1107.7-3042?².ØãÀ@;R¤ À:Õó‡K¹<À<u¿î¼@v™!N¯;@éœzõj?Âð¼@7¨Ž?e1Àz*©Ò?Ÿ˜<æÿí¥@»^ÃYÜj¿ÛMšÝ¼^@¿ÝǟÑÁÿ¿æ}‡ ¿ìTÃ;S"%?Μ­ 6Á³¿ïÿÉy[5±AGNfsrqPKS 1105-304?ï«Æþ_Iš?€Kš;	ª?_BЕÊN8?`•­äzÏ?%æ\«}£?}8ñ2?ïÊøÄë?~Í«9¸?NW8?`vjøæ/?v¸º*º'?wðX´Ib½?îùK©ª<? Ë`<àï?pÞm–?sYÝþ`¶)?œ¥{JME?Š®ž;ÿZu?ïäh>³T?PVlԔPó?'$ϱCZ?7ßà×0m?j&›q ,?Oå'ò
{»?ïW£^ïq?ŽæNw3 ?o'pIûáâ?m¶Ôr?'oÇöê§?ŒI§¼ÒA?ïŒì£Ä?‰Ôº‡Éï?Tµ—ÉWCÖ?eÊÂb»ãþ?Š.J)ê–)?‡SÉ ÝÖ?î;N9/?•¶'ΩXÅ?}©üû­"?€¥LÁÕ?ªœå
}©Æ?"ô™fæ5v?ï¢úçù_8?rN¯¶
Þ?Cõq©kÄ?@›Ðui'ƒ?†õ2"C?qÅ®c´gAGN4FGL J1107.8+1501¿Ò_¬wd@O‡EŒÒ
úÀ9À]''N#À<<Ò@ª;@+ÍcJ¨?ýÄÔ`?ù?¶šCžÌo–?µÀf#z@By<,9@0™)^"?ïÆ-vZÐ0¿àÿø¾m8"¿Ýw¥Þ¡`¿Õ7Í¡³ï[¿áp #‹öC¿åšíV°AGNbll3FGL J1107.8+1502RX J1107.7+1502?ï¼m­h¿˜?g·'qðq?TØø'(6?>ç¼fG§?|'ë_øù§?fFÀ"ÍÁ?ïbºC‰?Ž[¶»ç—ì?qí–£k?s¸'àëøÂ?ŽZõ˜=¼?‰e(ƒá­?ïB÷¿rNÛ?ƒæ'æò?t°+ƒrÚù?wc"q—?'tý3ñì? 3Ä*d?íyõiE‹G?"'¨¦«9¥?Ö–âö}ø?wy¿{)èÄ?©u]ý›¨'?~aâ¬0º?ïya釡'?{¹?²ãŽ¦?ieŽ{‹˜ ?V/ßH©×Ê?‹N"#Ì?xÇ+Í5!?îP.¡Ü'Ä?¤tŸMÞf?‡Ê™=i?ŒŠX|½?¥
o'•t? ´¦ùõ?í0´B?	ÐìÕ?|ß!Ï
Ò/?v°.Ê¼?¡:¬ö®øš?Œa@¯­?êBq$ì…?œßV+«?±8Ã;L³í?'¨ä¶¤Ô?¾E);ôn?—æ\CayyAGN4FGL J1108.7-1844?·êçhûQ@BçÁß3ÞÀ:Ò
(ÝnÛÀ<kDTæ³@¾òÖ§l?ÿž\\!i?ÎÏÅåýËG?ÂU½ ÝE@?ò®²Jj‡]@Z©è"8?Ò ~:Bœ¿ãOäÿÉy[¿â˜¶DË¿ç¡â"o¿Áô×ÃJíå¿éø@~AGNbcuNVSS J110845-184505?ïxfDÇI?…ø$ÂÁ«è?^ídh©E?W`ý½ چ?ŽÎ_è֕?ƒæ2·Rá%?ï'÷1¶lŸ?ˆŠ5x‡Ñ?eøÉ×Ü>À?gÌòÃ1¾?‰Ä.û¬c?"±ìœóŽ?ïEÿËý™ô?ÓA'2	?e,5Êbr?Y{ɺL²?"š…|×'?€4єóû?î薼ð`Ñ?x͏,'¶û?eçËEV(?OêÕÿ늝? %%³«¯?xY‹Jðö?îÑ	ò¿r?'î"_Ýz?réã´ö?dõ5géç? Ÿ#–98?Ò­K"U?îÕe6)v‹?œËƬ; ¬?s;LcáG?z"@½C? BHЮw°?™ð
'é?î~aQK?™T•§Ü?wrÎ¥áB?pV‰ðjñ?«É×P¾œN?—³ƒipJÛ?싡j.®$?—îÅìr?x¬s?e?mÓ2"œ
f?º-€8A?˜3>iôÅ¢AGN4FGL J1109.3+2411?äø±ÆÐÎ(@P¶'Ìö¾8À:?9ÉOiËÀ<g¨"1 Œ@ 
¸÷'Øã?ýwM©Öþ?¼çýÀ4¸ï?¥uø)Çύ?닫à.@[¨ý?ëÄ'¬í3u¿Û懞olI¿àÔN¡MÿÖח`Ú5k¿áüÄʟ̿̂ XÐ{®AGNbll3FGL J1109.4+24111ES 1106+244?ïÛ¦<@?W­k?Hî{M`?3¯ÀAš_?nE(ë¾û?U•ï¨àW›?ïÈoæõ»?u,Œ€'Ï?PªÑä…?T֟OaJF?wÃâhK‹?r_6cﴝ?ï‡ú~r?jQ‡œjÿ?b™?L@ô?Vs–›ÿ?‰[ƒ0ª?f	I
³?ï?ÿýÚ?qÞ½DÁ?€*7S®Ê?]³Û5,žû?•'é©ÒL?mì‡‰"?ïÀ¯Ã3¾?p…Ä?×{½?Z6±:§Å?K©².¸3?yÌQUFÔ?l…}Íʇ?ïVœs,Œ??rëÅI?d"µÇ‰)?j¶/'e?'ªÞþb"?(ÙîxË?ïÌiz—÷?'bœïšÆ*?o ÜXÖ?dp.Úå?˜'o×4w?€8ÄNojï?í£xy¨&i?ŠáN›
áD?"RöùÅI
?wAZ¦ß9K?¬üìæwã?‡ú˜¨|JAGN4FGL J1109.6+3735¿ÅVIZ3t™@PŒ°á´»^À:¶'néšÀ<…ý	«zm@ óÿ'¥?ù,Ø:¿¯?ÐKs›Ù?ÈTµyt
>?ø7ó÷´$@	àŸµg€m¿â¢X_g™—¿ì곝PÞ?¿ÑO7
XH–¿ÓØLÝ©=ü¿ßŒDý
,T¿àcŠØûAGNbll3FGL J1109.6+3734NVSS J110938+373609?ïÝu5%¦?‹4m¥1î´?:0Ás'EÖ?VS†¹é'?oD²º7€î?ˆt€pØÏ?ïØË
à¶?q®Šy6"ã?AâuÕ[?If%úžr ?q^,3ü8 ?pêÎíÇÅ?ï‰(v>K?Û·ÕӉe?Sv›:Í0?Fÿž&qïn?‹G&®`=<?‹5?½Þ®ˆ?h£a¬i?P~²µw?4iÖF°Cf?Â ²ŽC`?ha¶+0<?捻	½¢? iYˆ²l?FÒ÷áuW2?SËf¦>Kø?…
g'×FŠ?Ÿ¾bK°ŸÉ?ïxêޖà?‡ÔI5+šˆ?Q؋CØÙ^?Y5›í'·?Šf³ðVÄ?†DZoY¡~?ï]ëv8Ê?\•õM´?]¢"sû´?X5¢{;õ?ƒk	M?ŒÇÄA'Y?îšâÁ3o?…ÄTW¥?_úcK½b?NàZvB?¥gbâ/ ?…ŽŒJP±AGN4FGL J1109.7-4814¿ïÓ¿Q±oñ@&êþæûLÀ:³þËLš
À<ËRyI˜@øS*I¦@|š»É.?Êh'äÄeJ?Á	pT§?óøÜP'`@í}ÃOJ–¿çÕ\¾Fø¿àPVXÍ÷¿ëbâ¸Ç\K¿Ý©àc­y¿åzэ%íпïÿÊPʇAGNbcu3FGL J1109.4-4815PMN J1109-4815?ï}¿ó9aå?¨ð"D&	O?bnÌ_Âó?tö)ÌÞé¦?‹ôòˆô?¦nÝÆS½Á?ï5õªçtÄ?¡!îÏAva?dÈpdž'‹?ov&Áç?–¨<—†4? ßB°Ã?îãüŠ]ö?Õ§
‹Þå?sÊáoÅs?uòâ£#?ž¶taIô?Ž<bÁG0â?ïK$2±¥v?qÕ)Ãjõ?]P
2¡¦?@ÿø †Æ‡?"Êd¥Œ?pU[ê§R?îÎì{'œ?¨ÎÅɘýÍ?~ày|´?"H¯PK3?¢G	VH?¥Œ)±Ž´·?î$¦Ž°Ã"?²&"kñÚg?t>†~®ä‰?)㉕Ö?«-ÆEuà??±u뉘ž?í €)AS? ±ý y2¡?…0ä{—5?'Ã9ÆY?°Uâ%µ­]?Ÿ@JX«Í?í±Wb+]?'»eeBL?xžN4?c¾°Ñ*í?°ëdèaþ£?{
ÏõsAGN4FGL J1110.2+7135¿½¹^+À‰Y@E°U2a|À:m«|ðìÀ<­ú4ää@ ÛN?üºØÿ
6»?ºŸJžê	?ÀÄø(e¥@Ÿãåî@æÏ¥DG®¿îfºI<‰ô?ïœàÁ q:¿È¶ÅúJ´Y¿ÚI›)'Ÿ¿ç*J+Ú¿¿=ç—({AGNbll3FGL J1110.0+7134RX J1110.5+7133?ïìèAƒ"0?Qק"ü¥n?D'S!T¬\?9ØMM1\.?[æÓõº|?LEÌñ:?ï¤Ø'k2\?ƒ€§µ*`?cñ$wÝ÷â?lm'Y?Í–Sšƒ
?{¥™ß'Ð?ïškf³ñ½?mÌôãç'?`¶ÊDʺ?a'ç²Lµ
?…7s×	´?da˯½Þ£?ï#‡0áI\?p‡±Úîý?ŠaÀJ™'?g
»nœf?Òƒ×'?fuxqH?ïÖÎ>£?d©˜ÏIÒ?_iû|¦¯X?XŒ7ëXšø?i|ÃÐè§?[[¤Šq/.?îëÜ¢WÙ0?ž[>¼" ?x$阱Nƒ?€tðæôu?œ{1F…p?™ªÚu0T?ï<öÛ¿?UÏkÀÉÛ?o,w;zœU?lwÐöÖw?"{•Ÿ$x#?|¡	<ü?îk:ƒ?‰¬s$µ£?›!3Mכª?Ê'lZ»?¡¸²´SÌ^?{"–žAGN4FGL J1110.5-1836¿Òp B¯kØ@CÜ­¡À9ñb‹"À<0îP«?@ .l6˙?üo"èbT‰?À7¡?Æ!w±<y@ûB±Á¯@š#SAE›?êéTWp)^?äšs´,Â׿à´uBwHâ¿Ú{Ϥmˆ¿ÞìTQì¿çGpÂ_ágAGNbll3FGL J1110.4-1835CRATES J111027.78-183552.6?ïôrêÇùB?Bgdgî?A«Üß"V?3` tê5²?LˆxO–
?7etc?6?ïÕ´ÅU¤?tQÓñ}?Kªzuý?Uÿ‡)ís½?q°­Ü˜"?o±5îŸ$?ï³HáèŠ:?r'Sãr!Ñ?\¸óæ:?V®ÉNêì?*à¯$ì¯?pfh±C«8?ï!rLèT×?qã•ٚÎ?yéËKõw=?W"U[sè‰?•WCŠx§L?pQ0¬íŸ°?ïí7ö]â+?O¥c%áà?R4UQ‰i?De–ŽkÆ?S[ô3¢P™?B.ÁΙu­?ïw Êü?Š¡»"$Á?b-jÚÞð%?h•%I›>‡?Œ¡
<Ÿ?‡+ÍØ_x?ï€Bü»
C?~d鸏®×?iïw­o¿?iôäpeïL?‰sb÷fÁe?zJa+Í»ñ?íÎhsºj}?ŽCxÚð¢?Ä\C€eõ?uW'kRP?«¨a¶èÚ«?Šë#Y^[¤AGN4FGL J1111.0+3542¿êÌc#'z@PÁ)^ž	À;Qχ'0À<ݐ8ÇǪ@ BÞ£Žåá?õ?\l¡?Ý8LA÷ò?ïñð"<jê@ϵdÑ:ñ@Æ¡Íš¨?ï¦Vv.Z†¿í³Ç™kv¿Ê¨# 8Ü¿ÀœaJÙ«¿èÁUj• ¿ìcõrÞCîAGNbllFBQS J111056.8+353907?í 
¹(*?Åmœ"_ü?Vd¨°"±?›?ãY{þE?²êÆÀ¿?¿¿#¨	?ìDßGxº?ºÊ˜ðì?°.Z}ÇM~?µu'Ðé?«bÍ
f$_?£®ñ{4?î+¥FZÉ?œ9É'Øé?" Ž·Z£#?…R@Ïí?¨‡ñê¤?™cƸ†zË?éÒçÖ4÷Ñ?¦oC­õ?³^ûrƒ~p?¡}²º%K?¾	ÅÞhx?žŠüêÛl?êök/§"?Ãÿyù§\Œ?£u—b­€?¤UÌÎï}?¾'"¾>*?Á;î²iý?è_»ýG?ÇŠ•"o?½€øð¹ˆo?Àð	0?¾'ü

a?¸ÆÜ°Hs?ìœ\¢B_¡?¥«›`u?yJˆ~-?‹ð7`'?¶þÈKÍw±?¤ôKà¶á?ã`[q¸ ?ºW@G‡—Ó?¿›d¤3?a?¶Œ#'ÏK?ÑXoòpJ?¶)žš®nGAGN4FGL J1111.4-4624¿íóÁ»;Ø@*œÜD9À: Ô`?ùÀ<-±2ã@gò'"ï@Zp?Ñ_H$†òù?ѵ"2E?ýü+_)[C?þû0ˆ!¸?ã¶i´Ï€¿çàæ_E	õ¿é–'q¬ë†¿â¡¬­O"¿îÁ
F9 5¿ï6¹ÐpÆ<AGNbcuWISE J111127.39-462504.0?í;Çà?­fc³Å?•OO†k™?"²˜ÑÅ?°Ï­çTC–?¨ñb/)v7?ìE.}G?¸û«§wÎ?¢
G\Ó*? Ä¸l¥?´Ïëe¬;º?µ"ŠxÛÏ?ì—P¡ƒ? ÅÌKŸE?¡ê™Ç~éœ?"³=5?²P.•–®?›?è'Û»?êÙÌÍ2?"ŒÓø
Y?¥î¤ÜðeÁ?f')d‡§?¾?·-±Ç–?'ï<'õ™?éµ×¥K‡?¸äÌb_?¥ÈCšòO·?ŸÉÉ[Tï®?ùƒº	P·?´ëâZ¶V?å¢/†;ª?ɑ>)9ø?»98xõè®?¹¯eiˆ§?ËÚ¥¨p¡ÿ?Æ*©'Ç(¯?é5x/;¬Ô?¬o§À"S`?±,€?8? Ë[0óÖ?Âb‰–¯Ò?¥…*fyêN?ãWDC*l?§ÖӏHX?¸³o¯j…=?œ&('LL?Ó$›1"Ú?¦DxwWqÎAGN4FGL J1111.5+3455¿Î
J¶‡'@PÒ¼j~ùÛÀ;pZÇ̲ÌÀ<¡`†R"ø@"Ç~Õs•?ûr
—~?ÉüšoØ¿[÷7	B?{yïÃê@€(R¯zW?ÖIë;LÝ(¿ïþåþ÷í7?ïÿüÚ±'Þ¿Öøè^£¤_¿Ýî2BrkW¿å»l°Ú(AGNbllRX J1111.5+3452?﹐À7c?ˆ0ÊàÿØ¿?9mõ®½?,A=óº§"?€Ð`MC9ñ?ˆ5°½¬Ü?ï}߆ã´p?£Ï_gk5?_Mí4?m×úÓEaß?Œ§{oèT?£‡J<³;a?î5LÇ?Ó¿È;õM?T"ãJÉ·?=ÇÙ4]ôÑ?¬
(Æjº?Ùú5E?î=EÂú2ƒ?ŽFˆ¢æ¡?eՍ×Á·ä?X-ð±¶ú[?ªÎJïE%W?Ž'¡ë³Óé?cYÆ?‡$+ƒf|a?Bˆ.­²F?7>Xð;h-?‡©¤LÒ ß?†Ü5S&¡2?îÝák¯o?©"Ó[à?i$9ŸKÈË?€P‡µt>? ¥¯9"?§ò'Ûùý?ítô{½e§?¢Ú%'9AÎ?[#³PáW;?Xӈù<ž?³ëÍVÖ«?¢ÔLZçü*?êñãž†¥?ªJm,yz?w¶®¡jRÂ?va"5J?Ã|
ûº(¹?ª+þù9DAGN4FGL J1111.8+4858?ì`~h÷Ìf@Nu>ÄaÀ;׳¾
ëÀ=µš &@!Yy²s…3?ð4Âkñ?çÒÕZ::?ßê^bá̎?ôéËº~@ò00õ@^?ïø÷Bl64¿â~p·'©¿ïÃC·õf?îVų-¿Óm'©èò¿æjmAKúªAGNbcuSDSS J111158.89+485701.4?ïjÅ_?·1ö7ÎO8?oak¼þÙÓ?'N
"PLÃ?š†ªû?³'ñ‡ŸÏœ?ï܊tZf?t$5oHÆ?BŠgéÚ ?\¤×èœ?nÒñÐ'8?qj,OY{'?îÿËÁxË?ž@×±cW?uCJå,C?}"Aß•?¬G'›¾Ï?S`Œõ¬?ïêÖj°M?S"WED®?ã\"ÙK?!ê]žøì?dB|9©õR?S½+~7Û?îùÀÒ(èh?¤둖½]?zlô/ŸM`?Ž`w]0g?š,¨¶ŠC¥? f ¢5???ï‡fÿr?–©¼`õ·r?PøkZò·é?e¨p½{wÐ?ŒlÐêX?–&,^"á?í'?öÿÀ?¢ç[§ó-ò?xP÷;¥»n?ìÑë?µ@ðÖAj®?¢"ÑE¼Ô…?ïÌO$%œ?qŽýŸ­£Ê?&ò‹Açß?;:–ö¤-ñ?y ÝH¯—?q|Æk\	AGN4FGL J1112.4+1751¿ë‡V¶}¼@PX£/D'*À;%ö4À< ÷ÞÉN"@››``"@ÄɅðoi?¼Áw녿´ÓœIÍ('?ûdÏÃ!R`?þS…~»÷¿¢-ï7Я¿æÉ	><Þ¿åü8§ç:¿Üg&Ɖ½¿í	}£~?çœÂñAGNbll3FGL J1112.6+17491RXS J111224.2+175131?îxùv#æ?Á¾EÓýK?tA´«šÚV?r'…Æ/?¥è2Rô]?ÀÝ/à1Ge?ï€r×
?ž‡
%é?¹­¨?'ɳ§\±Ï?"³o
?'F˜H/;?îY([¤ýŒ?šÅƒ‰ð­?{¦fÌØ?€
<ó:¸?¦~w4Ö&?™\7Žõ»?îñ?VñÃ?'gÌr?…L6Ò^þ?mߌÃnë?—1ù³pìb?xGÎe?í@¡©;*×?¼ÏÉ8B½?ŠþÎB&·?Ü"²´×
?²›ót‰ó?¼uM
h¸?í§"ø8ǃ?²ØÅrs7?'ƒ0IêqÞ?Ÿ,'€S?¬Ì8ZíêÝ?ªÌ²æ:¿Á?í¥0Ú?¦¢i'ˆ
ø?"q‹ã?S?€+$·4?´¼¤û©Wr?¥¶í'óçx?ëÓPGú–?¢îuÕU.?¥tý¬Ç?–>a³¥éœ?¶«p6Tíñ?œ&‹ÒSôAGN4FGL J1112.5+3448¿§Í*0NS@PâBؤUÀ9L p¸ÏÀÀ<!@ÏÓèJ@Œiƒý%/@ô¡ã6ï?ªÉSE¢Kš?›Wߺæ@$ñÃ&ZÞ@eMÌg¿Ó¼¦Ä¥`ø¿àÉqޔ a¿çˆ	¹½%¿éœ
V›¿éMnÂs-¿ïçâ!´†AGNfsrq3FGL J1112.4+3449TXS 1109+350?ïèS……ˆ?ZBž¢ºo?PM¨å†·?DH¯Ä''?_Ù¸T$?Tî?bêNŸ?ïÒZßäE~?p´Ü/hi?JÅ-q'`?Q|#€OÙ?s]0\?l×êó‹v?ï¤_ÒÝ?{"èÅ?jæ<ù?p"xo^Ñ×?€.Š¦½f¤?tDùb6ÀÙ?ïëûváçD?Eà˜.º®?N5A´F¨?6y‹è(Ëõ?Xù÷dêR&?=TÐßz}5?ïƓóÅè‹?u¬Ïîø–3?^µ†q~´?XUgX¥?uļîå?r­ËõøBY?R$ª?Š\ºAåª?[ªÕ">/?h
™›Ðá?‹é>	µgT?‡ÿÂßù?ïYƒTê?ˆq¼jZåõ?wÜ	/C"x?{ðrê¾ZZ?±&V•ˆÊ?'ñä-R?ïʸƒrCr?cùMíGce?d®Éruvx?T… hè»-?pLYn·ó?[GP£êÖýAGN4FGL J1113.6-1920¿ïû¶r'@Bë ¾Q	À;›r·®À<"‰†üÞã@|€3>q?ú''Y4?æõ2ôD
?ØbëóÁ{?õú%zãËí@VɩתK¿¯¯EAA'›¿ìä>ÙY£
¿»ÔyŒ]ò¿àMt'yè¿ïúïàM28¿ïÿÿ>¹úAGNbcuNVSS J111348-192252?ïuýÃÃAf?" M`,¦×?a"ê3:?kú<-ª?Ž:ª	¤$ª?'¦EÃfn4?ïÎ…÷•?yIPez˜?I_?èïf3?W¸U#1®?uÇÔïsÔX?u¾¨"´×?íV_!£"?£[L¯j˜#?—"&Ÿb?"ÓnÚ±Å?®ÔVºéùÃ?Ÿú¨C¸é?,"mc?n˯Vre?Bƒ}ËcÑ?6_cmÂ?‹íÄã *«?n3IyâÂG?îº!õ{Ë0?§(\U?qÛ»CøÖ?uxšÐa;?¢"i@É9i?¦9À{fÅà?ï^l'›æ?˜zå,Ç?b¦¾z?tÛéƒero?'ݪݽª?•¢eP2F?쵙¹òL?¥ÃrÎ,2?'E@C?"u?(©œü?µÁâÁ×¾?¤–låò½Á?ïFúeaY?‹ÛÇ-Ôä??{ls¶?I#:NÓË5?y3	Ò¹?‹¼[ë¾AGN4FGL J1113.8+1528¿ìS+ºÝ¦@P!¼ÓZ…ˆÀ:õ'R}À<˜s%³@k֒ÉEÚ@Ì_¿ƒ8.?ÀÞº z^k¿¦âSÁÊ?眐úŽ¦÷?ùræ‰âA~?ï›îs¿ìCÑ¡ð§¿ßJ¨/^']¿ßæèArf$¿äw4cn¿ß-¿ÖÅAGNbll2MASS J11135586+1528058?﷉sˆ
?€i#"ƒ¯?VàË|S¯H?J×Øü&rÙ?~ƒSé=É?jg߃¤ã?ï"}$\Åm?—á
†_œ?{Ku‹¨®J?ÜÎ&.
?"Ý~äàÖ?'Nzæ^?ï.+!ú=?‡·²lú!?o7	à÷›?ps/"øVÏ?–Sº¯lS`?"ҝϼÉÓ?µ'ÐU?€¾^P§?ŒJLl?rŠOÍéE? CBJê°?z*¿Ù¸°C?ïUÿçèmM?""Jµ­?o`%S|vð?bC]ÿßê?'Sþ]R;m?Žœp£&\?íòÞ|Ö?« û¦"¢ì?Š=³\â?"à¹o¡V?ªQÇ~ù?§GiIeg?î áCt?'׆_E‡?u]©í¼h÷?l~CçYz?¤c(±^Ž)?'›–ºW?ëD™•õv?ž&*'B?¦,aÈG?'À‹ËУq?ºÅq'F?˜í½¥jò¸AGN4FGL J1113.9+5523¿ë.=øU‰@LX[žŒG¡À:Ÿð+oðÀ<ÎeÅV¶Æ@ïÑÃ=­@]'Z
7'?À)§Ù£Iò?¸HÈEÔv?ù@ùª{i-@¨âºtÛt¿çuB!b¦?°'×5[†¿æeçñr¿Ô:Ð`€r¿ãž"Ք¿ï÷އŠMAGNbllSDSS J111356.29+552255.6?ïÚèlC'Ñ?"©XìŒ?F\'Ÿvʯ?@"ôq{Ãh?o€o:Dš?"¶¹eü?ï×ÐbGé?r¡%¨Pٜ?G6¡ýÿÐç?S†­·(6?q0úb øÍ?nK‹ ÝÝ£?ﯶNä,?rctË%w?Vbl½]»?UŽdrøpl?F©­»?qMC̨М?ïµÜÅ,3T?[7R´Èì?m§Ž¾]—?Km#ÃeU?v>*Æ7g?U¾¼Ûìd?ïËç¤`êH?rcÚ.È?Sãum°Ö¤?JÃcþüâ0?uP-*E?pÅTÂ&ç?ï'‹"?ˆ´	kë_?[ÒjÔG?dúi¿i"i?‹ÿwsv'?…+þ«?ïb÷G¹ká?'þ
aIÈS?dݙ$1E?k[Â]-
Ç?'cáÀ"?fNSl†?ï5ƒ—F$Ÿ?xšù/¤?","5¿?i/‡óÏÿ?Žr…ôð.0?r%²±ã{\AGN4FGL J1114.5-0819¿àÍAý®õ@G¾Cªy»®À9ԙœØXÀ<+£<±@<Áz^?ü@CßâSG?ºÖ<!ÄJó?ÂL;ÂÎÇ#@­·®W–À@@à$ÃXÛ?拝'uß¿çƧÿ¸ÝW¿ê)!¯íï¿ìäÐ.Ë¿ï¢£Y6¿ë¾hêAGNfsrqPKS B1112-080?ïë¢I¸Ó?aÿ?â(^°?Un¯:¶¤]?UBh"
úš?TV"ê?TSšƒ¼Ê	?ï}R؃Óù?‰¦"ÚW?pÉæKJ—ƒ?uO^µƒ·?ˆFV»ƒç?óyÞ¡?ï'S8?'³nU‰?el
‡È׺?oOáâ)t?†aèo˜þº?€âb®ž€?ïJ©Ø«þ?r±Ù{ŽÆ?‰!¸¦>?mdæ)l™?"]\ßwqî?aŸˆÝ8ô¡?ïÏev"õ%?uB1œ½âå?qçngç?r:jKƒ¥&?]u%*å¼?[•,t'"?îNRgš²¸?ªC5'âÅ?†iÝ¡?#þtÖ?¥€vD]Ô?¦³K¯Fx6?ïNÁ?a%?‰®"7\¸"?oAFª´ù	?rã¨a­¡é?'?¯Eçæ?†üÜ1mö?íŒ'ð©?•nÕ;Tkœ?§5l¦úÞ·?'e1ò'8"? 
 ×pQ½?ƒOÒA~ AGN4FGL J1114.7-0248¿ìG'#©Rt@J¨~8ëÀ:EÏÞ²À<)œ1úN@&¹¶ðl@òÊ!÷¡?ÃúûHáb?¶y"˜€•?ð™šäó?ÿàTyá?ÖBˆCa¿êÉԕ*™¿è±5Ý\'ü¿çӄ¼¿ïý¸'gù¹?ÊöÖ-ɒAGNfsrqPMN J1114-0248?ï»èD³Ÿ?w^-"bý?q–Æ·|?pʛk ?pâüMÄÉ?js™g¶?îjÞSÄ"?¤"XS]ˆ?"5#‹;3?–õŒëæb?ŸoúŒI?—³jó`VÏ?îvz!H?•µ6}÷nå?,]"'H?‹(4¤ê=? ÍF Fˆ°?r¦Ü:bƒ?î‹ï¾Ù?…XÒ6ë?"ňf¿Q?{"D•0s?™¼¾a¤?xœÎŠ˜œ?ï:˪&É\?—j°À*;¹?‰¾=ŠG?"‰Ãq‰ä?€;úÚva?zôZmÿHà?ëÙ¨»¦9?»wûµÔžä?¥âšCòw?­¬vˆJüM?¶AlÞòá?³pÖ|Š$?í*¸R?Ÿ$ÀŠ¼?™Ì *xÂ?'ӝØ_Öi?°8R4ˆÑS?—OM.׺Ú?ëûlro?¥íBäE?²€=ÎÀã?Ÿøнd}?´È"^ÆÚ?šA$cAGN4FGL J1115.2-0703?ÑÚ'ä@HQ^	À:XaÀå8À<Lk"ÌÐÿ@ò;"™¦@@"Eð?ºÒ6™A?¥&¨$:¶¤?çވì£+ê@ÆâCV–æ¿æƽêî¿Þ.dß¾—¿åÎÆ×ÀEÖ¿à-î$nt¿çéŸ"w¿ÙÀq_=ÓAGNbcu3FGL J1115.0-0701NVSS J111511-070238?ïßpz³Ç»?^"¯|Î?F*"Ø,ö?4F'ññÖ?kà1ªQ?[€Ç—*ð?ïÖ\ Îgé?q¿ŒÎ €?G{þWRZ?Pð°e8Ã?qâoì	¦?m.«;èñi?ï´Wà*'?nüFZ'ùÏ?VŽ:Ʀ?SÉyÅ	¨)?€)—ý"ôö?m!Åö
ˆ?ï³&ʈé?[ó†.?d`lIÒÎn?C±zÏ}Ù?|<d€¤Ru?V·LEE‰î?ﻦtÑì¥?oŽg|05?W™¨e!Œ?F\È	¶è?|F[¢F?ln.¾
¤?ïuC8'Ó?/‡'‹+?ZÃæa¶c?cÐhË4(?cLj^?ŠõpÇø®{?ïx(Åy¥?}™º›XËÈ?bT¹ç?_-—ÀŒÒ?g\Pôö?zÝt&¥Öž?ï(†•õŽý?yÿ­sbò—?}.Õ1s‹?a×âû›jø?"©aƒj½•?u–ro¡ŠAGN4FGL J1116.6+2915?ì'<Ë.ß^@QB­­ê‰À<Kl»êý9À= ¤&ó@#¨©Úî¤?鐗ÈAî?ép›Þî7?ê~e`¬é@"ÄæN~@üiÙ¿ïÿùSt?ê‹ùæ/t¿ØÞ|øy#?ï¡æڕl?Ì«IYæ%c¿Ð2":¯ÔDAGNrdgB2 1113+29?ï:"úY?¥~¼ã9?~ 0ìéW?@·mN"à?•°¡:PG'?¡ý µYÎ?ïª23¥?•(e¨:2?`\¾ÔßéQ?åB¿Œ*B?\Càƒ?Õßç?ìZçQ!?¦Üç<³¼:?'8µû^Ñ?'ºÂâ|Ý,?¸šš>'ßW?¥ ׳RÓ?ïW"Äü'?|.þfØz?AÀüü#eë?G€íRÚã?‹Ž	ã‰?{â[ŒÎ¢?îüáíÆA˜? ¥SC ?‰í]ËiÆ?–[ä¾lH?"maƒ>?•JoPN›?ï7Þèûxÿ? ·FU^],?n|>ƒ3±?…ڎ¶¤ˆ?•4›¯9 ?šöã͕+?맩V|Ó?¨ÕÙMÇ[?)¶qf€°?ŽüfK1x?¾¸I¡Î`:?¨j Sß0?î¨-:m0§?ž"f§aÅ?Q"sÈù?gsÂlã?¤ðˆÄ®G?ž;ÙcÍɑAGN4FGL J1117.0+2013?êk€«zÜY@P×j~ùÛ#À8úùåܞÀ;ï*¯ÖòÀ@9 Va¶~?ÿH"¹7Ē?¤œ|^0ž?Q~'œRç?±"÷¦À½@±pÿÇuö?ϗ#k"ù¿ããpè gê¿áE†òÍè¿Õ掿ËÝd¿äο€³ï†¿Ð.feÍxAGNbll3FGL J1117.0+2014RBS 0958?ïøMË~²Ò?C¦"Q¾?#K`ú_b×?ö¹ó·Ü?Iõú¿6'?Bl!Àús?ïÜ^ãe? ?zqˆtSr?;«ÖŽ*2Æ?G%AË\|?pÐȗw?y¶–…,:?m'÷á?…ž£BŸ\?Rùc¸é˜?ECn¸Kë?Œ4ÂÌ»&?…{ҟ¤¿u?ïõÒU*‡q?9Êҕ?(HµN÷?ô>>0?QR>¯¦Å?6I)ò£§?ïõm®õ	?L8Ý·%aC?*¥ÃQ`f?":,&ÁP?QÏëÇÛ±?I•Z2²BH?ï X=ah?ˆ¼Wz3y‰?J™—FHÈ?Xwàû?†@WGµWX?‡t'OؘN?ï7ñřk?Æ^FýØm?X»'N³Æ?O´HdÒKj?—vØtã¼?˜±Ø£ÇO?ïé÷ïÁ™?R¢Ryˆ!?:àTš²¶?,-WšÿFÞ?b¬ãªâ$Î?Pç̤~:AGN4FGL J1117.2+0008?¾ÊÌƱn'@Kcí¿‹›ªÀ:÷k:
½ÉÀ<Š|@Ã?@ ¤É'PÑÕ?üº¡6F
+?Ë­=¾§p?®|>>ÿð?â®q,"@µ+‹¿îÏõ@‰]?ïév†oj¿Í$¨ҿDžþ²"&›¿éÃl2š‡?֖K›ßÄ÷AGNbllRX J1117.2+0006?ïÂ9
ãT?qô˜"F(š?FSÑv‹®?7z?Š¡g?|ûü¥?qLã
24?ïÛR2k¦Ü?q;$Ó¥Ø7?D6`Þ]?PqÊìÚú?o MjOÉ?l¨ ~\Ÿ?ïI¿»†K?†Ü§­¥âu?eeJKl~È?aë2»l…?"_@¨Ü?†D2?ï˜×·âYý?dyJPԁi?b;–—þ,J?F²/3´?…;,oØQ§?bPñhdý?ïs5녅Í?…¡¡zäw¹?WÁ!_V9?MïÊÀ0¾þ?0‰)?"´æÜUqp?ï'Ø&$à?'f…è{Å?U¸è@%
?`TX0Âý?ŒÂ,ëˆj?fX3#Â?'·Ž]?"j¯àÓ ï?rJò—äš?p÷¾K
?£ì8ƒYå?"PÙ,Ç(?ïš&ºÝj?€$3½Oõ?p³øW¤ˆ‰?^|;Èח{?™_½—¦?~%g![AAGN4FGL J1117.2-5337?ïÐãò+t@ÐO±;`À9ÜRX'hMÀ<HjÒܱ@¤ëg†ù?û1GÏ¢j?¼+‹tõ¡?Ì´ªV«2s@…Ìe÷@ºe+'÷?î©¡ÙY"¿ä
~q ¿ÓØe1]¿Óޖ"ì"¿á̈¿V"¿ïÿ'âH	.AGNbcu3FGL J1117.2-5338MGPS J111715-533816?ëYْOoÌ?¡üæ+SÒ?¯	~áŠÞ'?°6…qEFï?µ¬sûã+W?¶Ì''AË!?äp ³áÌ?Å3£	sµô?£‹.r´F|?¤9ӎÇ~e?Ô­XÊÒy?à¨Er¿ª?ëgÅÀ$Y?¥ž¨£×óã?°a|´ÀîF?ŸtƒEÖ_.?´`ULB
Ø?žDÇ4{j?ê<Ê—ñE?•ÊSÔFv?¤þ¬ô¹Q¥?|à'&Cch?ÁÍ,£ÌùB?"'Fm¯?ä¢Ê{Ÿï°?È<!a'.¢?ÅÇz%h¢ß?¾ù¾®-?Ç­[ìž`?»ÅÃ¨Ðˆ?×ã¡´ñ?ÈXÍ1ݯ?°Î$E¦?µ)}2Î?áô·¦¹¬x?Nj®6+,¡?è<-:JԐ?¬¼÷ßM˜?¹Ñ<¼&"ó?£óO÷ÇÉÄ?Â&¬¸ÁcH?¥B,-,q?ä~–'Á‡l?§0PU³Ü?³.Y»rh?"•'Íi·?Ò7=iÏ?§@þŠÐw(MIXED4FGL J1117.6+2550¿êa·šÇ¨@Q@9Õä¤À:tu;ÄÀ<šk‹iU.@úGtª@Í]…U?º]âžÆ)E?Žê¾¶oÏW?Ôf˜:@YYBfê?î†òBR5¿âÂÖ>e–]¿ãæÅÒÈq¿ãµDD¿æہÁ
̸¿Ù¥W½×žAGNbll3FGL J1117.3+2546RX J1117.6+2548?ﴘؠâÛ?™õ
\©?h°?™
7?™.*îg½"?y[sÿ6B'?zŸ›jÄäà?ﺭò°ÐÝ?y§Ü¦RE?T-i'î?YM5«D$:?}¢;f£ò?uvçaÔSz?ïyIàý9?wÄҝ;M«?i
£[]?oHüâØì…?‹jÞå«?qÀ[^zPª?ïjöñÉ?jm?ì"¬>?}7€ÖoYõ?\`€ýx1±?†¦ƒ`<î­?dE$F6=O?ïmª¨_°?…'fAŒ?oy\kEˆ?czãhH'‡?ŒÕ7Žéeª?ƒ#üÂÜ4?ïF¤)•{?'+ÇÝcmÅ?c°—`§=?jlª¯÷k?"ÉXˆ‰$L?
Þ°mÿ4?îíX?ñ»?ŠK•ƒà?vD›Å«¶Ì?q0<??À¾?œÃ×–Úé?†fë[(%Ö?îGÏý®Áõ?ˆ£—õ)¸5?•yºQ@?{)oð'ÌŽ? ¼CI£.?'±Ô÷²4`AGN4FGL J1117.6+0217?æ8ôxë׳@LBŒi/nƒÀ:Èût€À<])4¬¯÷@S¹¿~Û}@ ¶fXúm?Ä\HUYMÏ?B»ÆÇúl?¡Þ.ÁUí•@gÕR­Kþ?ïtŠˆ×¿â'~e'¿é´*¿qD'¿ÕØO¢T©%¿ë8ë¹4¿ïñÂàÍ=AGNbcu3FGL J1117.7+0217PMN J1117+0216?ïž	Rª®?|,Ãçz¿æ?eiÁ *ûª?W¨%j$`?ƒ#L½s?Ÿ?yF‡ÿ‹aƒ?ï×?.5"Ú?pÓسΌµ?DÄ.B&Ç?OÕƒºfn?qÇã+¥t•?lDÃ#	Ö?ïn%F.?'ǙƵè?eœŠëÐûà?iãJ$¬Öº?xõ?~ï¼>ËÉî?阮Xìw¯?b¤Û_cC?h®&©˜q?N!/Ë?åÀ%)ô0?_U¸ÐâÍ?ïTÀŒ!¶ß?!°é>‹?tîR+‡?iþåÇÇ3Ä?`rèr=?‹¨jž­ O?ï{j*ÚãÖ?‰'«Õ+L&?V6"'¤×î?_
÷miúÂ?Ž^¢ÅՉ?‡>2`gƒN?îÆ- Ä}•?'Ù1þãqë?oÎÜäø]¹?f‹'t?¡ 8)ž&J?'½k}Hød?îúé¸mÄ?€®ûàq~w?ƒk,ñëR?oG"´ö?–í2…Ô¹Ø?z'z¹tfAGN4FGL J1117.7-3650?ïì'n…wV@6Y~™cõÀ;òø°€fÀ<"ö(æ©@Ҏqó7p?üãx«ˆ¤?Ôo›-îOÔ?Ó.¹PïÝ?ûUȤI @}´üvˆ?ïÌʳíض¿é0ç"øoé¿¢è&šs‰:¿Ý[5ZÕ¹…¿î¹Þ]˜âe?ÕX@2õö'AGNbcuNVSS J111758-364918?ï
»šÓÞí? G"¥ öÌ?u|þ³Âè?@Ò4"µ?˜éLñ[ˆ£?™•Bҍˆ?ïnHvÖ?—ÀÍÀ0¿ã?€_]kºA?™'›ñ…?•bˆ1þ"õ?"<jS*Ö`?íÑÑf'?œþ·Z^?•ÐÊÚŎ?¬	°CYe?¨ezw½Ë?–n=½Âò?î&œó|u-?"ý 3›?…¤ÿ?iý¼®oˆ/?¨-0F¼v?'	ÌѺ%`?î
Kâ›Yý?§²V&°Ì?"5äû,/®?yʝ>µŒ?ªMȗ«OF?¦pÑÚjԑ?íËó¢¾JB?¨ù:	®X?Ì¸wLµ?"xc—h·°?ªÚi™Pè^?£†ÑÞx?ì‹p.™Îü?¢ˆR&@ñ?™¶pç_$r?'K±Í©?µ6âO¡ñ?ž"W@|Ê?ë=òÅÀû?žXŠG^?'ýŽôj™©?Ûc¬å^9?Àȃ
¥º(?œØÓè¶=AGN4FGL J1118.0+5356¿¢ºýÈfbj@M¬ÿ§ëlÀ9†S³Ü;À<"û¥'l@"J"ú?ü‰ÔÊÈÏ?­Ÿ¶¿Zð?²?Mȵ»ä@_íQx™@‡k'–Fÿ?ïÐnýäœÍ¿"
ñ)¥…¿àWŠáÅ¿×h^ùŠšù¿â.î%)¿Ú½_œr¼áAGNbll3FGL J1117.9+5355NVSS J111757+535553?ïµSNå?"õÖÌÎüÝ?Wg—?Ypž‡ÄÌÐ?Wó—?'ð£w±?ï‡k@0L?‡(;k?msór•J?qÏ{Óµõ?†È3
‡¶?'ÖP>ä?ïEÔQ•7Ï?†È
tp?qWSÆ Ã?q…´HXJ?'ï Þȧî?ƒ)ø‹êFí?î\"ÀLòÞ?€'¥þ˜?'%˜žz‡Ž?p—5''C?¡#÷ª;ÀZ?z͝ì¯'?ïf>¸l?%yåˆÖ4?ièµr}u?d òú@ö?;-¹²Ð?Œ¦ãÈ֌Ù?îÍ oª:"? Ë7Rèÿ?Þ!°O¸?"ÙÛ2~
?žTi£W""?›[8Pw"j?îadi¿"Þ?—8ÄuC¹?ƒs(	%?'eÀ»|Ü_?¥ï\Ü´R?"Žõj"/?ìrëû™Ço?—V'{…a?¢iòã7W?ˆ»W¨Š,§?³3§öN[?•= %x*KAGN4FGL J1118.2-4634¿åÏOë>–­@*«nø_»À:ZëÞàÌÀ<3ˆ˜`´@¬Q'M›@TªFJ?Ñ4òÛª5H?Ú$&»U¬@1[µˆ@(t,vÖ?ïövêB(™¿k»Ý2Âí¿çòCŸ'Æ¿æcçeÕFï¿ç]13~²Ž¿Æg³'ùÄýAGNfsrq3FGL J1117.7-4632PKS 1116-46?ï†`½ì?'oÝWqr?_MaË·¥?W V½Ø?vú¼RåØÈ?'P"EØ#?î:1ÉÉ·?°ÈUBŠeµ?õ'
PˆP?—ðVÃëp?£â[³Ëm?«äü'Žî?í½Ý"¬[#?ž¤ç,SÙ?–j,B79?ew§¸?¨ínu+?—YÓÚ'ì=?îÊWzmâå?^5è᪦?Œ=Ð)ªq¤?lÜ÷údjý?˜–( Þ†?}§ƒœÂû?ï³óï?WH?|\hÚ¶¤ª?kR]=È`u?i1¤Gßpö?x\Ù×m«Ò?tü'¾XGÄ?ìbV"ê¼?Á]¿"¼ h?¤	¢Ñ\Æ®?±9ØT²E?µ€ãô!I?·®T®y?ìbÍÅù§?£–\1ò?¢s:SEÉÏ?•OjZîŒ[?³¯ô§kÆ ?ëùIÔª?êÚ¾ÙUW‡?¥H$!–h?­–O…³?•û'å2…u?º^ᦒj??£§…×`sAGN4FGL J1118.2-0415?ﮃ¼ô£½@I²@(äüÀ9¶<ËbjÀ<z¹ÚÁ@ †ôü@Ù@ÍG¤ç?·ë'ˆþì°?¶¤?	ˆ?ù+õQP@|@BeU¿Ú rÑ®³Ý¿ãá01 3¿è—è¿qšw¿çœ'aï‰:¿ìÓfQÒ[¿ï"Í®oêAGNagn3FGL J1118.2-0411PMN J1118-0413?ï÷†ÒA«Ç?GäԊ+²?1ÿ÷SòÖp?'¡i¹Ûm?HäºÚ>cM?D7â
Cœ?ïá!£ÇM?kŠÝ¢0¹«?<æAi'Iò?HkS#Îg€?kA"@•W?gÍz/Â7?ï´gP!x?u'=A/o?[÷ZÌE?Vê£4•‡?~ëú£|Ê?sm$_MË?ïø0y‰H?2›DW[{8?/òν(?é'êyž?G֊>×p?/fØÕ+Y?ïôD/¯Æ?Kl KF#?;_G­Ðrž?0c"w†'?PŸÎÌ]9?F,¸Øƒ
¦?ï8"íQ
?‡ˆ:{ÅÖá?RS¼>V÷6?`–8;y
?†g±Š'ì?…ßð]ãš?ïxwlaìÉ?'^$M:9?eÉGŒO'à?f¼ì±ûÚf?ŒoÓžõ:?€àe,•åN?ïèmhI{°?T_9¼.Wù?JJ¸"ýnk?>8_Z5P?`ÿéÂïXß?Pµöõ$ç¹AGN4FGL J1118.6-1235?ï%7‹BÏï@F*䎊qÞÀ9öñûÀ<;Æ*\}@ÛÓöeM@Hæùž¼ï?¼±;aU"?Âj‡ÃŸÒ@	Ĩa³@8÷¯#™?ïÿÿÊPË¿çîG;'ô;¿ê|Vþ–¶¿èӃÕâö¿ãÏò@Ϩõ¿ïþ,UÉ`1AGNfsrqPKS 1115-12?ïÕ@á0©?v
Mk*¶Ü?LåÇ7&²?P
è§:YÅ?qÃՊ|?t$ól'[?ï¦ÛÒ?{ÿà‡¬?bM9Š©"?eG‰ÑÚc?µíj'¦ø?xmǎƒ÷?ïO…Ï7`?'޵闚?qæ5‡€ý=?xcóxä­?›<ã÷ª?'C÷ݎêS?ïlãÂvvn?o¯Ú-Êqà?'xŽ¼ÛÍ?gržŸ:1ó?'N€—C@Û?`WNs?ï¹ñf'?~½sÂ0Bé?abħ/Ò?ea}.c?zÁ"ô:]?y³ÎÃ?îç`&¥?™ÎèHåë?{–èa˜>W?ƒTuM4S?œ.Bˆ²À?"怺)Ñ?î\UQ§N?•ièvØkÀ?~;´óz~&?€z®ø/?¢bÄKèÛ?"ˆ»ôäù&?î#b€R˪?)6ùôõ¡?Ÿÿ,8Á]?‹gR\‰½?›"›ÐM]?~î"©äûAGN4FGL J1119.0+1235¿í'Ùž8Ý@Oø·`,'À9íÝ{p¹¦À<Þzt:@%ÿµØ>›@=ðüVþ?½M6êwØ?Í^#vҚA@3xî(g'@
~w)W<¿ÂäÏw÷ÞH¿Ý8e˜º¿çÊ3ß3W¿ê¿cW¾-¿ïþÖj€˜?î§<_VÒ AGNfsrqOM 127?ïȘ§£"ç?pô¼¤©u?m£ÇÊ¡OÏ?fÃdŸk?iЄXÊ?aÓ>Mo?ï²Ô.§™?€XR…À•?`#K ó™*?jö¤%%‹Ð?~"Bô*—?wsɹç~¿?ïúD̅!?'ä¼òr?	…~žZb?‰ºl^3MF?»ô¨×ü¶?…Ü.ñXh?塀Ö´?g㙷0ŒE?i7JÚBÐæ?R:#cóŸ"?oã#}?cIõ㸟?ï‹!›Ù?"µN[ ÅÅ?|"T4 ö¤?z:
óS¹V?}ë#]Õٞ?yÖIžg³:?ï	ÂdF¯?¡±pFG'?v÷I.9?‡$‹s½Ç3?™FnöÄC?›X"úO:F?î!p;…ö?œ,¦†s?žw8†[j?•SB	tNÛ?ZÀl¡{×?É–ü9›?îÒ}'âQU?‹@*"2?"ùËL]ë\?uí÷Iå?›3h>­¼?… ei%zAGN4FGL J1119.6-3047¿àT‹ÃÔ<@<ÈæŽ>óÀ;c…LXžÀ<´)3Õðb@"/sš×\?ü8ÇÃ?ǂ´eLàÙ¿˜Du?Ò¼Ú;uL@'®¨—›¿ÕÀæå|Æû?ïÜE É
пë{;	ÁJ¿µ59È£T¿×ö‰Ÿ%Ÿ¢?țt$¿ýÜAGNbll3FGL J1119.7-30461RXS J111941.0-304652?ïµv‹fiÛ?{
"÷­í?BҮ锗¯?5¼é#mW?u2@øÎG?z?Ê¥Óu?ïÌví‹øá?vˆÜÃœ?G9å¢;4?Pñ¶œÏÑ?vÝg#Д­?sõ i8?ï:ÌGýÖÁ?‡˜W¸Pl?`‰€F2P¢?`¶¸ñF&?–•Fþ¶½?†ïŸEç&&?ï|ôíÓ,¸?uò»¢A¯?YRè ^úø?D:>±õšy?˜gy袌?tÉ]ö$Ã?e"hä?pÕBûœÖ?Q±%¬(é¶?Hø +rƒ{?ŠÜAÜY·Ë?€àދhäÓ?ï}Qõk'?Œj­¼Éñç?Tƒdïû?`Ž%ŽW5º?Ž(?WÙ?‹¦ÅùŠJ?îáY$4ä?Ž^rá?bÑL«'¹Ô?`úùvr#é? ½Xñ Ñ"?"Ð9»N?îIfE%Æ[?'ÌQ#ß?tˆDË¡ª?jeá× ?¨Ø"=€†?'Ÿ®(fÜAGN4FGL J1120.6+0713?ï€/úˆ`¦@NV0U2a|À9ä(rÀ<P)Ôà@˜à¯à«?üÉçÅv—6?¾Fa8T/W?ٟúdŠn@XÿI Û@ˆj$aY¿éŠÐ=š•B?Ð6¢~oœ›¿×>adžæ
¿â¸J"xÈi¿ïÅ<¡?ßjÊÄ^êAGNbcu3FGL J1120.6+07131RXS J112041.6+071335?Ë¥ùø¿ë?Á fêל?è)‰øM?ÿêTŒ?žêÿÀ^?–¶N÷ƒŽ?ղɠg?Ì:L	?âÅGÙn­?ÌÚ%ýâæ·?¸Ž¯?½?®»AÕ¥ró?Æÿ²»‡2Â?¯Œk<FÔ¼?çR؁®7Ù?±úÿÊù¡?·iÖ{è7?¡#q16'?å'Éč@Î?° '²#ç?Í°›Ú¢´‡?®[B
å­?¸z)À,{?•LѺ†õ?¶4,Qšã?±3{"Þ"?ìW@¡/å÷?µs(Bs«?œG:Åk¢?–èTr—?Å*–°ÊÒf?Å郇]?çzD³I6?Éí¢'3N?¹Ø¬ÿÒފ?´Qc¼©CO?µw"˜¨¥?¥Â Î&‹?ê²d²ãü?¬"Íøcò?µYcJÊuý?¡¶ÞL¥@?ܹεQ¨a?·¼TnªD?×|žê™ïÞ?ºë)š¥€?Ǔ$À(ς?©ô«ÎzvêMIXED4FGL J1120.8+4212¿ÌF ;ÁU@PŠk΅3±À8ÁA÷TðÀ;¦. |w@ ¾ØÈ.?ùÀ¿xPt?¤wÉ¡Zii?§`®>@eŽšbv@tmoïüþ¿ç'E'ƒ¿Ï²¼•ÇýۿՄ½A¿h¿ÕKí^'²u¿ÉHY`™¿Ñ+¼üKAGNbll3FGL J1120.8+4212RBS 0970?ë‰!#2¬r?ÍC«›¤¶®?"àƒˆ—?•½µK*A?Àz"A.°?Ë(‹¯¡è?ï`†Çɝ?"Þ<ÞCý?q"(?|8yüÞ?uÜEÓ®D?tŽ~O¿›?êH²BKý?­…[¥ìXñ?'`eЧ=j?óíBÑk?đ*<ó ?¬büä˜÷?ë;u7 ¼_?™_#J3µ!?•À¹ü¸
R?ye¶wÿ Ÿ?ÀZáx[?˜-™kK}'?ê¢Ç¼ÜX ?Äh±Ã»?ZˆnÜ©?"R7Äã*y?Ã@Ãе÷?²âu«}È?î;˓øÖý?±ÚüÈ¢w?‡»øHŽ€?©":—îƒ2?¤áWÂ`l?¤=eø=¥
?遑?Ù?­¢°á¸*ú?'ºá—þò‹?{n"åV?Ç¢_p¨ßˆ?¬r0DÒ~#?æl>Ø
?¯¹—…«¼?£¾",ògÁ?1;åùÝ?Я±Êy±?¯ŸVꮛAGN4FGL J1121.3-0011¿ïÑÀeúõn@K"Q´þÀ;ËñºzÀ<œdÐd1@ Hƒ}Îaø?ÿ"à°«.?Êϝ÷øµ?ŽÚÜs͛î?Å£øSY@ҍٜéÛ¿ïÛO¡ÓÏË?ïý…Ò<xV¿ÛeD¨P—¿ä6"Ü¢¿ÃÛ-¸Ÿï¿è;¿(Ÿ[zAGNbcuMGC 0019706?ïÆ
Óî$?s¨5é›åy?O'½»º9?Z†Ô_†)þ?yQ	!ܳ?mÌ)d)£?ïÕÌUñ?r¶Fí?@ˆp߅"?J3ˆÀpÚq?sì "^?qIIr¬D?ï1µØQ»?‡¡²>l|t?eŠ×>Ö¼?iÕ¨dë	?—§±>º?†qv……u?ï…p¨a?jÖº•	?[4	¶Ném?F:%6ø¥?‹={ò¥à‹?i}B/£?ïnßå6?qôV¬²?_¢G¯¹Õ?YG½»ÍÏ?ˆÆg@B?€	x¨5?ï|-("XH?ŽùÛǾ${?U®ðxX˜?]œó·æjf?Ž>óÀ2ˆß?F¼Ï›ã?îtÚ-̊?"Aשˆ–?rucã4?r±Ð΋R'?¦pîuV'Ü?'òC¤"Ÿ?…ø@Þ?"ʃ·Ôü?k7¾˜	¬;?`ŸPo[ö?¢ó;¹yÞ?"eiHfsÄAGN4FGL J1121.4-0553¿æ%ÖқT@I9PüqÖÀ8¥Q­DqÀ;Ï×ð}ñ@¡sÕB<@x"¡¸?£À–2±Ù?Á£~õ©dé@Sžã…v@ƒaòåæ¿ÍýV
㘿â°]ˍ1¬¿å*Ú~çÆ¿æÀ–]¤öÅ¿íƒ|V'³Ì¿ã$A"àAGNfsrq3FGL J1121.4-0554PKS 1118-05?ï¸;çrüˆ?tAHÌ®ä?p6—çsßN?hÁ$ù5ÂÏ?s«tCüÒ?h™íÂߺÅ?£šÿ?'HÊ´´.?dmŒäÈ?mÖod2?ƒ"'<ß?}«Ê YÃ?îÅ·ëzs?œsJ&I'Ø?"M^òšŒí?Šº0S_Ÿ?8Y…#ã,?špyöÍ7'?ïÊ~Î^"­?]Z"kÏ~O?cç×F ÁY?MVg§4?pÌ­GÂPŽ?T@NGYÝ?ïaT™'?Œ4ÒQ¶?ïfy4Šþ?z'·–è`è?‡ÄÉ£@š!?"mó*àûl?îå‹Æ$ðƒ?Ÿ¥¸¶ÀF?vÓÓ9íô?'PÌwšœË?ÎRNzŽ?œoÄMè(?î>ÒÉčA?¤N\•"`×?'´'9JP?†sWª«ü?§e¯rAÛ?£S"Ëª_?ïb©üÏZ,?|
⩞m–?}"¶VÀ`k?kÂOÌ?ˆ"% ÉDÊ?uÿªÕ·AGN4FGL J1123.1-3233?êóÆ,¹`M@:¹Ñ¢£YÀ;–m•/À<žÉ¬†Ü(@Rž˜†ôü@óý]ŽP?ÅÁ¼"…ù?‹†ù?Èòüvރ®@‡A 3fµ?î=ï^òÿ'?ï§$f畦¿ì)õœÏ®ÿ?"×Bz+Æ¿ÜKóÞßsî¿ïÿõž}.)AGNbll1RXS J112318.0-323219?ï³Ê@>Î?}UE–´û0?Q7Æ¬9?CnΘ•"Ó?€æ‹,ü[?|Wsn^šÒ?ïãÑÞÚkq?k"m§ü?=µx½îó?GB×tGÒ?hŒJ}\	1?féî¾µ˜?ï=$Á*'5?‰AlÒ~L?gÙ9Óoƒ
?ob‰¿?•`@£y?‡K›<…ø?ïÉ;Ipü?]ÙÐ4ÆL?]û±ÑC¶?IÐg˜hV?sãnâOW¹?WÉs+Ie?ï˜ÂÙ{SU?tý.'.?\éCÝó¹<?Wv÷º(ˆÊ?†2!0}'?O;`V'?ï®^ûÁŠ'?"õ9KÝ?O—Bssû?\ÆyÄå"C?'vgé?ƒlï
´µ?îÄe\r"?'0ß|ïî$?oÔþ¡:Š±?sÍ*†Œ"²?¡¼ZO1	›?íø,÷Û?ïoâĆ?xþýXÁi?ukžë?jR`Øå?‰Qù&Y÷f?sµ+ü¡;{AGN4FGL J1123.4-2529¿ëÌ$á
ò@@£Þzt:À:´É.4À<Q¤Æô@?ÿòˆJ¼½?Ë,Xãñ×s?Ó¢šÛ¸ù@j[¾l·¹@«_ð«y¿î´@ÿ¤n?ïý_;Ϲç¿âFr«G¿ã¢$'–H¿çêèÁŸòú¿ïÿß~€8 AGNfsrq3FGL J1123.3-2529NVSS J112325-252858?ïä?A3|?^0Nó÷<Ç?Oc%='sZ?Iz½³ˆ&E?d
÷A?V>HÇp?ïÐè¯p4_?u†Ýñ¢µ?Q?SûYJ?Y¾ÔɓÚÚ?s;Óeü1â?pMÆñ7X?ï:ä‰×t?‹À/k¹¬?y¶šTÙ6ð?|'þ®ælº?'5Ù^^7Ì?‡Ã9KUÞ?ïŠ4ž)ª?d>€Š|4Í?rgs;I†?Q™ƒAdž?"?Ÿ'Õ?_.™Û²½ˆ?ï«I«€Þ?s@«Þî÷ë?`˜Î«dÁL?U¸pŒÁ'3?v]ó¹P‡?pr¿Ÿñ'#?ïvø
yfÚ?ˆÖLo›ú?bx¯"|Ü6?j{ªdÿÉM?£Ñ‡ÅÒJ?…'ÏƵA?îÍ´Qo£?'ÚLéÇí0?€–ÆPó¢?€¬.`×Vw?žFIR"Ó?8ú"Óƒ˜?îﴚj¾ª?¼aB?Ù¿*Îó?j	&6ûà¦?™ýƒÙ?yÚ©Lí=AGN4FGL J1123.5-6418¿Ã™E˜:ŸÀ] Å®À9ªkµZÀ@À;)Ì¢Ûb@¥'—H±@EKc¬?Èaq	,¤y?¼ðò›éU?øyìU(Q@¡¨ä»+?ïÿP3:¿â¶CÞÒõ¿æä%®æ2¿ì	tÞNTw¿è(úà†h¿î–JŸ‹vAGNbcu3FGL J1123.2-6415AT20G J112319-641735?ïŒÍóŠÉ?‰øõ¡a¢?+D—ÉxQ?&dÀá¼?Œ_p¶÷§?‰VJ<ï]?éú™
O^?¿]IdÖw?pjô^ñÛÛ?vüìÑ÷?ǒD)"gÅ?¾LŽ+¯ä½?ëæÉå*«i?¦øô)$?‰º(~{~?†uYãC?½'kÊJÞÃ?¥
ᖙ›-?ìò®µÏI?'™*@ÂÔ+?o‰ëâÍÑ@?N°g°o€?·r³)ºBï?'M¦5.?íÔ¢rljH?ª4EVK¨?<èÓå?7"Ãþ·Ër?±>WqŽµ?ªØ¢–À?ãÚÒýú}p?ÉϪ¤ê?wÜŕ¯U?ˆ€à°Çm?×î>'á?Ér†Qµ¡¯?éBÉÏJ??¯A_~¾?•->7ÚH?'+({2÷?ÈQsþû?­'±¬­?
?絜àSšå?§¢†m»ñè?ƒé…4Ώ?l´_N_V?ÏêüFѺa?§a9`ˆAGN4FGL J1123.6+8028¿´~F
ø³}@AótÝÛÀ:Øý›²yÀ<ÍK
P¼@o*|«L?ÿ³vŸ™Û?ËO äüïT?Õê{´V^@>À·pD@ÖèÚt€¿î''¼¨'?ïùx&'JÈ¿å‹ZÜÅhT¿Ù'D:Ât¿î­¿jäz¿ïóHa˜¡LAGNbcuWN B1120.0+8046?îžûÑ¥­,?¢ÅäbV¢?ŒÇ¶Ù¨?"jŒv«?¼ª`~Tv?¡M0ÔAò?ïï'rّ? *£PS^à?Š@§­1½?–Š˜3Ø
?'Áº3¯ï?‹¾'Zœ_›?î0?u-K	?—CQ÷®?"ÞÒiáô?‹¯ïºê?£z™Geún?"))w¦2b?íÿå±}ą?‡,ìzÅ¡"?¥¦ÀŠÔlÅ?ƒqQ¢@0?"µÈ¼Vcã?u[Òøٚ¹?íŽ	s!?§Š}"pä?šô3‹K6Û?"Ɇ".œw?©¥Tö—ðy?£QWÀ&
?íxá‡l"?±¼¢ßȺà?»'IJ?Í?¥=PUša?©"ZPañ?£.c>'Y?ìØÀŽ>á?£š>!?l"Ó·!À?'áµèßÞ?±äÌÅÄY‡?Ÿ…%΃¡¯?ë€Bq$ì…?¡ýÕ±·mv?·ƒ$5#?ŸÅfV?5?¨õ†è•j?$jräAGN4FGL J1123.8+7230?ïoچ§W%@EŠn~bÜnÀ;œ®¶aP}À=¡'Œ_@!¹üøä'Ì?øÃæÄŗN?Ê-˜),A?ɀ1©k@óH+è¼?õöA»6L¿ïÓèë"³¿ï¶R¢dCv?ïÿÂWþÅ¿×î]@L÷¿ßx`cíæ"¿È*ýD8êAGNbll3FGL J1123.6+7231RX J1123.8+7230?ï²ÜݖZ?'q[Q}S?N¼ôLÙ?D²ZáýÌ?]/»Az˜?~lÚ´v?ï.~?öåû?"ö­é)FB?x¬#I?Ý?|;èÙ³¾?"/*?7±?µðô;ª?î‡y[&˜?•¶À³ô?¬?}ÿóc'?€¿'ˆ]D?£Èkæ™VÈ?"ô0	?íÕ",‹àZ?Žû]Õá-?'ÛLµ™ä?s'PË-?­÷
?êd?ŒÔI%;b?ïbq§b/?ÿï¬Gz?`9᳛ÆÃ?`o3•áÚ¢?'ªŽÕ"N?ŒŒ§ozt+?íÂh]•$?®EÐ|F?°/>NGË?"o#X²-?¬mn[fþÉ?¨ÃÿäEG.?í–UÊaãu?žqÑ:æH?"óóð6»&?‡
Ä< í?°®Ó/Åóó?›»°%êMÑ?êdL¥lƒ?©ÌÇôiׇ?'²eƒÂ‹¹?nÃÅ ·Ú?Ä8€ºz¾?¨ÅàÌ{AGN4FGL J1124.0+2336¿Æp×tÃJ@Q~Æ"§À9ìú'è},À<-:ƒ‰ŒÜ@¹ö¾ëv@Bá¹Ãۍ?³ÌÕ±!öu?"Tµ ¥?Ô4ªžP8@ž{Fó.‹¿í'ó*ö?ÌÒE݄Õè¿ç$ŽŠqÞj¿ãi!Œ—¨¿ä
':ƒŽ¿çø— B•§AGNfsrq3FGL J1124.1+2337OM 235?ïÀf†O?wE¹z71?U``¡® œ?I"g-0g?zt¤ð¢Xr?ui‰dÏÙ¹?ïÑ ³--O?w¹àq|h?IHœgGÜÚ?S
èÎó‡?t'ÓÆ'ú?tI.ւÝ?ïwùk€?%Å¢5?f%m°,7&?cœê¯£Ð?Œ²&;$¯'?~Ø(L`?ÈS?eÑç큏?uÀÿ"pÎ?X€Š9Œa?'r¹ÑŠ†2?a¡¶Ÿm?ïkçù½µr?Š'~ãό‰?gì•
œŒo?ZçVy~$?
ÜIcî‰?ˆ—£RÞ|Ö?ïyz8fŠ	?Ž(Iù‡æ ?Wµ ¾*g?aê_¦Ê?Žª½ÆY$?Œ
~þ¿ñ?îÑ êyc¢?''6yÚO?xM7‰?w
 aÁ³a?Ÿ¸ò"s?ŽF±ÈÁ?î¹aQ÷{?ƒ `&>)È?¡âü)ªË?xê|æ{Ž³?˜1òêŽkÎ?|h#çÁ2AGN4FGL J1124.0+2045?ï
Óyus@QEy¿ß~€À;Ù¦ÏãÀ<¢­\Äüõ@ iZA"ö?þ*ål[?ÍÆ^ˆ¦?´¦ùS"{?ìzšï°@œ¶ü%?ïã_0пÔ3Éü7ôc¿ßƒ~O;R¿Ù*ü˜lrð¿Ý|¢gô[¿ç\ß¶´]AGNbllSDSS J112405.35+204553.7?ïâNÀÇÒ?\ÿ®°
?5T= Ô?&™ÓH1(?k·‹'S?[ŒŽñø?ïÌґ»\k?qÂ2	%O?Hÿ¿*Í¢f?PH¤Kž?vv¿NZé?o]"ÅDNV?ïƒ:c~Y?t¸€•¶½ñ?]m+^ ó?\'Å룧?‹y™Y'?syYâÐ?ï[)¢Cië?pþçÒcÆî?qäÖGa¡?S|) »z?UR"ì•=?p.EµÜ8?ïÏu™½´_?hï™:WŠ?@yŒ§âþë?2ځ¤þ?v6©)WÞ?hÚûî1N?ïoGº:	L?©ú‡?[Ëä'"?cõåY¿nª?ZVÂí@"?Œ¶ÂB†í'?ïɯ¥¹Q?…pø0k?eÏ6Æ^?_³ù&Ôùj?šŒãM£¿?"Ü@Àt?î5bº½ý?‹2ôwü?'šIs
Á~?oø¿ùs?¨AûchN?Š	<î©AGN4FGL J1124.4+2308?îC»#,*@Q{€Ü3rÀ:ã¿Í
	nÀ<]RÁmóù@T1I#4@bÁ–8?ÆM8`C¸?A±=é/Z@È1ÉPÁd?æcq>†£s¿ì>!£¿¿çà¾áý‹‡¿Øˆ¯üÝ`Ä¿ÞyÌÑý8¿ðAGNbcuCRATES J112431+230745?ï¾Üe,eË?z~jü†?M‹@ù{b+?DÀ< =?|àeeŸhÿ?yA;v[ —?ï±aŠÅ§{?•ŠÃ–VéÓ?J ¦A§?OødÏé.ÿ?'S>‰>?•N¸%Ê	¼?ï0­ÏSZ?ˆ½ü­î˜Ø?_Ž<1LN?H×R'øÃ	?—ñbJ¦V?ˆ]bL«s?ïhìžVö:?q@ä
{åò?gȸªþ´7?Næüj¨Sô?ÒªLé>}?p]q*•Ù?iz†?‡!!(gÕ?Z8þRƖf?RD‹DÌ´?‹ÑÅà‡"?…å^zDûÄ?ïJ…–ϲ?šíäŽNPµ?Xa–?xÑ?_·ýciÆ?•8Uîf'?šiIYäT?î;·¬æ9?–
f$"ï?láì%?cHYÙbÎ×?ª€b9ř?•'ì<Ão?î
´Hœ{÷?Œ¨#2$¹?ƒr[0Ž?p\<h$z]?ªH$«Þ©?‹ïÙbÀAGN4FGL J1124.6-0809?ÝkL }ʗ@Hv <K	êÀ;MFÚ°À<tò ›ìZ@ AêÜs@…Ù ð¥ð?Ï?8ÇǪ?£&Î 		ê?Ք˜B±@‰;¿HÕ²¿âBRÑ^,¿æbP1ò¿èð›.£¿¿cŸŒ¢»+¿è=…Ò<xV¿ïîåüH»[AGNbcuAT20G J112437-080643?ï͊Ҭ_Å?kŒÛN|†*?FpŸã¤ê?9²tVÌÁ?vl†šE1?i•?U$Â?ïÃ_•‰6?|Ä£ˆÝÁ?LÚêvŒ*â?RmGãºÁ/?z´×ó§n"?{"Ýx2ž?ïtãd=í ?y"ѝè?gºˆ«ÎÄ?qh ¨q¥?ŒØ"ø ?qKLâV¼?ï+£"ô¡?uÍ|×`^?n¥¯Gšå?SáŠ3̉?–¶å±|S?txč:G?ï‹Ç¨ÿ/?'©õr`':?ShŒV?KíÐùIï}?Š¡Røš?¨|ÏÌ?ïM<	Å#?,¦½s²b?`XÞE£%?fLՏ¡Æ?"McËÑC?ŒÿC‰Åû?îéG\5
#?‹#"âá?oÇ'õOv?mç"Ê`	£?žÞ/ƒwڇ?ˆUÒ}7y™?í­±zК|?'j²V)?'õÌ@z	'?q«yqÚ-¡?°3ºŸQ(7?ç^VI#:AGN4FGL J1124.9+2143¿ëםy‰?@QgÙŽuyÀ;
)Ù]ëÀ<³ó;Ì_@r,…o7@B\=îx?ÆÝ«Â;#m?¥ùìj¡ßc?ã|楻æË?÷¼¿øÓç¿íxmÏç3€?ïú¬Î)Ä¿å{ ŠN£¿Ô	.3ð¿çnýäœÍ¿ÆjVJpKAGNbllSDSS J112503.64+214300.1?ïYu¾·Ïÿ?±\"fh{?R<ě>Ï?bÙcWî÷k?"°ôT%F6?±'òH˜†Z?ï˜<œh?ƒ'ù⎐á?cƒF
°ã§?iF¬lÇò?…_JÒÜè?6ÌŒ¸Ü?ïHëOÞ~j?…ËX½ã#F?pâÙhæm8?sìî&úðÀ?'©ß«Ú`u?Åo{-é?î'ï'¹Dt?€1D—ˆ?"yÿC™<:?vH(z'ý`?š(mÕ;H?t¤þ…Œ0?ï?ÚŒ^?©ni²N°ã?_A˧µÈn?YïTéë±?–(Çü+Õ´?©]@È©ì?î·à¸Öº{?¦ub¥ä?z;]ìŸÆô?"ßîæȹ|?¡:ˆ¹Úè?¤5$+ÕU?îÁ8Wp?'wÄ.Yú?y†fjNô¡?z|º{è2? ½ï«Gç?¦N´2§?ìi­•úӛ?˜—@©¦¶?¦†¬4¯h?Aáþ‹k?±cÏøÅ0ô?'·ú<ªAGN4FGL J1124.9+4934¿îri¼(²@Ož@ÈG,À:ыxn§À<5ÜF½S³@ò5#ù.€?øNŒ¥•P_?¹ÀÖIxD	?Ã-ÄßB›0@)ÃÂb@
'AÜCb?ålk˜ÕN|?ïÝ`='l¿ÍüÖö¿Õ]°ŸÅ'¬¿Ôbºõ8§¿å_ü?EöAGNbll3FGL J1124.9+4932GB6 J1124+4933?ïå¤Õ6þš?iÆ\Êù|?Vˆà¤É
9?[.!ø4›ô?^-t'"¨?]¸R	Ì­?ïÕ|ÕyÕÀ?r€ŸªP³?K«¥dϧ?W9'ž.óî?qÏÀc·§?m‹Ø±t'(?ï7±
Š®«?­Ðqíº?l|$l/£é?u³™FKâ?•zZDþ ?È0è°L?ï>ȹÜsù?vÏ4Ï¡-¯?n¯™Éå?VÃRBG™6?"dRπ'T?uŠÿ¾_Î?ï¿êÖo…@?{§«(ٛ?pSV¯³81?mÕÂL\w?on|eN^î?oç¾_b?ïyqeÈܨ?¥É^Ëjâ?`Ќíà'þ?pÉ?oƒVÈIì?‰"×·?î¨j-~¬?™xݘiFT?}#£'÷½ª?ƒh÷g	Œa?¡ÔèÄâä
?—jŒ­?îOÚ'4ê?'S6Ò_Œ?{x*Tۃ-?l'¨­j}?§"XCÛC?¢Z+œEXAGN4FGL J1125.0-5804¿ìpBM,ƒ—@ ñ,'¦7À:M¼)çZÀ<zF"b@!þ"à$Œ?÷';ý?ÆûQš|m?Öw¦)ÊÔ¥@‡‰Fe?@K'à—ÚÓ¿ïýVlô!¿ï+Bn9™?ïýÀTïEž?Ð/ûZԷӿ͕c>"¹†¿ãϺ 9qAGNbcu3FGL J1125.1-58032MASS J11250388-5805404?֑ô"bg?Ã|7H–œº?«"媋¦´?£Cp.p"¬?ãA«Fa?Ä¢,šè¤?ã‹>•š?ÌO¬%7r?Œ'gK^eK?öœ
™?ØGš¦èj?Ìl•ï.æ?åÊè@ƙ­?°º=uxÊd?»oiÚº M?¥<2Rà
?˪ˆ‰&?«¦Ž4è?è<Só.?¯šd]·;!?~'c³µÏÝ?qL …'¼ó?͐oh?¯‡p?`Ɲ?Æ'vë§X?»P7ª*$[?¬õã(å?©Te'?è¦ÄNgÛË?ÀQ_(¦à?ÚÎ2—EÆ?ÏrŒ"»x?•"!³GÚ?¤¶¼'6W~?âN
ë{?ϸ—2Ñ?áñSµ¬?³ ¥¶å-7?À8ü1"?¬u±]à¤Ô?Ô.ڑ?²×8ä¬?á79H‡>‰?¼=ë¯!Qp?'w;?"'F턐9?Üp{¾s?½zT"ç…áMIXED4FGL J1125.1-2101?ål¡©]†ï@BÁˆ†aÀ9îÚøººÀ<:¿:=°@u,ŽSj`?ü©—"ÆÔe?¾OÓ@É¾?Ä÷'>]@Ôi
à"S@Þ跎ø¿ïòx6?ï>Áï#9¿Ò´ßñÙ¿ÝÑ·D¥¿ä¬;'}E¦¿Ýdæßr–ËAGNbll3FGL J1125.0-2101PMN J1125-2100?ïO?ê?¿}ûi©x?xB@á)w´?£æ<V©*?m/f?¹Zf§ª?=zNО?}§®òԘÓ?\E?æ6?eoYhè"?z Ò=?uògDiˆ?ïžP@ÆTõ?pP¿œøÉ?^×›ÃåÒ?bCüAi?"'¡!'?|駞ËúÃ?ï
¢s™?qX"êm9?ƒ©Ènvß?`ÈÓ®ì?"¿Ü°aà"?k=¨­_Öt?ïҌq_`/?g¯Ùïñz6?fYKa"®?^ž²ß¯?gCföÈã?YF§ò‰])?ïR÷/:Ã?–	
nW
?m+"ÆÄ?x
z?'û§©óF?'âŸÇN#?ïmÐݟû*?'"<XÛïA?h¡âþ9nÈ?k~Ï£÷­?ŽcOÍÌÞ?€FB`?î`ZCÿo?ˆ>5æXôj?'%@jùÿþ?u•»©9ûÉ?¥çZ*ŽŒ?ƒÝ՟PAGN4FGL J1125.5-3557?з¼Ý–t@7¾ÕϪ͟À9Ý¿zÔ²tÀ<:b'œOV@"A"ßÿ@ñÜPÎO?²ãÂË O?'B@c®Œ?ÒÄ«Á}œ@.~]Ë?ïÿ"g3¿áß
Q'™Ë¿à¬1¡¸¡ó¿â7´lƒ¶Ù¿Ùˆi[
lпßr&c$ÚAGNbll3FGL J1125.5-3558PMN J1125-3556?ïï½ÐZ à?M‡P(W°õ?-†£Uw?ðR»G??\ӊ»Œ0ñ?KóÕQ–Øt?ï渤Ý֜?ngхÙ?7·Ó_ý/?Fÿúý}(?fP`s:è½?kX)2"€?ï¦ÿáÕ¦?têº$$á°?Tr'S?P¾š"·*E?ƒ±Ç …—?tQ]—1W?ïՓŸ€Þ?RX'5âg?BðÛ!?"ÑP懓õ?rØúD'?Q±2Hx?ïádTÏv\?`K¨éypü?:ëݹ‡?+ºð•ü#?k>/Y?_­C1
'?ﴝ­
ËÇ?ƒ‡·¡ÆÕ?H5¤´é'?Zðî®3°?PZÝ?'4_ñh˹?ï\¢œ'_}?…#ŸHX
?]‡Uû%Ð?Tx"²Ñ³Å?'";ô?"É
.ú"å?ïŒm;—°¶?p"žq\q?X‰=˜GM1?AVu¾Œ	Æ?‰Ó‰oùä½?p!g;H	•AGN4FGL J1125.9-0742?á_xn@H¼ƒBÙÀ:"CïCÀ<_^4h½Y@ò¿ûƒ@ÖqáÄ«–?¿cÌ®…?`†K¤«?´É¼L!?öå§×ŸäŒ¿ïÌ7å?ï~•Òd¼B¿ã…Lò!¿â¾œ)¥ì¿ÙH¯œ:^¿á¥·]®1AGNbll3FGL J1125.8-07451RXS J112551.6-074219?ïWÔ]˜j"?Šh¡6îj?a''µç?Wـ%0'o?'ÓÂ*›þ?ˆ†÷¼ Àæ?ï²ÇÇÕA?|Åòb''?ZÂnFÓý¯?aÔC>;
?€!À9"?uÈ*YMÇ?ï"S#r)?ŠL"ÞB
Ô?r#"ëLÑ?q%ª›¶à•?—,©`žì¹?ˆÈã=s?îžÃ_:Î?~R**/-\?Œzbílà?qÂU,†¶ˆ?êb›ù3?vTèŒáB?îÏäén2?–‹î¶+ ˜?s;éL»|?jEkŤþ? š@ÛØÒk?"Ž"x«&?îú•Â8Z?zuME>_?r:¢›|nû?zà®ðZ©?œ¶øšÈþ?˜ôŸ–âß?îL†Êù§»?"Û˜Q!&?´¾=íÔ?€ ÍƂ?¦ÊcÀ2¤\?'X–˜S
£?ì«ü%Ø?–9¶¯ÿâ? shâªu-?ŒÛtâ(tU?²m«­ïò)?'@BIØd{AGN4FGL J1125.9+2005¿×âu´Í @QNµ ÝDÀ:ÁóTöÒÀ<m2ûÕÎÔ@ØdS爻@Âãú滋?¶h#ªÕM?«¬d!'¡Ù?ó¶îßFL@î[R×é?í.öWà'¦¿'ù†Fß,¿æôxþŸ3¿à2üâ>N¿æï¡ðÖ¿ïÿþÐñAGNfsrq3FGL J1125.9+20074C +20.25?÷Ìă?ÈÂbŒMf÷?zVÅG<'? ú@«]o?¢Y‡Û¬
º?Å"Úå-/¨?ïÜÑLcZî?m¾Î[È?C¼áГƴ?KâôÛB¬Q?n?{ïÕ?hž^Ù3øR?ï¾åš'×¢?o{Ú¤KXT?[AN석"?fÛbVb?y¼Þë¤Ó…?e}	¸ÿœ?ïÞâYã†?Nùò´?Yú›y²?=–ý <a‹?d—š_C?G¹/\±?î™vN™s¸?Ä°¾cÓd?~ A®aT?ŸE'PÊÉ?¢¤'ä!;à?ÁL&ÿÉ#u?ï™Vbã$'?"é¾Ð(ڑ?Rºæ½1g?^À^"6²L?‡S
u0?ƒQ€;O½?ïšY`?tÉ̓÷+6?_©Vê_<K?YT¯'#ãp?…ˆVÆj›?rø"»°?奈>'6ú?j3aÀà?qÈÔìh4þ?[gË(ýa*?{ñÝ-?bì@(³AGN4FGL J1126.8-3829¿ê3\qH@5uX!)EtÀ9¥Ìô9ù À<>ô±d¡@÷oV¤ýP@|½ÀÀO?²Êà
œJÏ?¶˜ã¼'Ž@aÑü·v#@8³Ík-?Á4âö.ðÙ¿ÝEÓÿqá¿æs	¿àwy¥Œ¿ä3ZÖk®¿ïüev|^AGNbcu3FGL J1126.7-3834PKS 1124-382?ïµr¥äք?o3¡
E?XKÄx7B»?H_Š¦'Ìs?3»íw)g?lêõí™?ï‹sÍ=q6?"ñç´:ÌÞ?nRc^Nô?|ó
æÆB¤?…Žsã¶úý?‹>f§…¾¼?ï'¢™?}''hl€Õ?hÕÔ ;Ô?jñÝ`ï]3?Š7¦*8È$?x<@°Ü,?îÅu%ún?u"ߙ$I!?ŽAŅ ^ò?eŒM·ÏŽ?˜<î'ÑJÌ?p'°S0‡ê?ïV§H¦.u?"ϐW˜Æ ?kR8Ÿ[K?]…îÌ8î­?'ÀÏÙëšø?'Ú˜V"\|?î¡àßm':?¥«¨%?‡Î2\Üjs?•ˆfêo3?ŸÜÊâ5–?šVmC&$À?îÇ»–w-ç?'Ä:ó?~'2[?|6@Kzì?Ÿ€¬¬©"M?Ž]][ÙMA?ì˜ÜXÂ0?'$Le‰F»?¥š&‰ö?"'•Ñÿ_É?°l	÷!Jƒ?ŠúÐàœAAGN4FGL J1127.0-1857?îã9bn¬}@Cɚ¿3‡À7s;dZ¬À;Y–¹‰$@vú«Ø5Œ@¼ô}þ•?"ÕÊCÒà?´ägH8¨é@!ŽGUÿç@ "ŒdQä¿Å`Ó)ˆ9 ¿Þožˆì£,¿ã‹à)÷¿ãèJ®kc¿æy2Pµ$:¿èžÎÂpRxAGNfsrq3FGL J1127.0-1857PKS 1124-186?ïÙòû"<f?hAÒmؙ?J*+Â%ð<?DbG¥'G\?o'y°-ÏX?e$@šŸ?﫪`ÄÄs?…Œápž?]ªHSÛé-?m§tflæ?`Ô!™õ?Ðõ'Â(½?ï°³º_Àc?†»<–.6;?v`šùƒÍŸ?ƒoP»É?qE‡åºI?vBÓ؀³?ïúFÒGe?2ÙEöÿÁÌ? ÛK
B$?D´_!r?BÞÁ°ï"?01ªR­ôù?ïßôSÆÈô?e®["y??÷Ô¼Ëþ?6Ú5	÷…?l±f"aV?dàªG
Ya?ï1´>FÈÍ?žbÔnS[!?hÞ9½®$U?}†¬ç³
?–­±à½Â?›³µÛ‹ÚÔ?惘gsèÁ?†8ċ˜vš?s´Õ{ÇG?17×D~?wö¹Æ7ð?{"$Š©]?ïòƒœÖ‡?PÊ-Ý÷((?0ß}Ô ï??*Ê;ìÄÞ?VÁ풖xX?Nô?ýôÇAGN4FGL J1127.4+5648?êRóÓw@Lbك"t—À:KÝþMxYÀ<ªþÊuÚx@
ÀaÖ	@mñf­´?¹A]˜a‹5?´ü‹+lÀH?õÈbŠ8ӆ@/Vôk!?ïÿäA2¥D¿è"d
ƒ ¿é3)Wèb¿êSi©¿æ€››ÒXþ¿ïÿþªJlAGNfsrqS4 1124+57?ïöڏ®g?Sœ)Ê\c?/s7‹T¿?>(ÎÂÛc?L¸ó¯©ÓÄ?NÿRY*A?ïÙÎN=`ð?p«ÌÜÖ?EÈD6&Cy?Pïu›Dý?p_Ðq[ZÄ?k¥ÓÂ=v?ïfÊU_i-?‰ªÈ}ù#D?aƒô»"?jAË¥Nq?'ÚJÝÌ?ˆ÷Åzx?ï딹
"C?C—Ú]Q;?Výù|mÇ?<Öïi'?Qؔ¹…|<?6[€£kÑ?ïñv³CA|?Víûóå@:?9A"Q;ù?>RVn?VÂ8Î,?SfpÔht?è¡a?Œ"m՞í?YdZæ#?cðM"2/?Œh®°¦'Q?‰¦QÌJv?ï*½éZ!4?Ï*}µ–?nÿò'þУ?v
êfQò?–ÈD{$р?o'yÆë?ï¹Ò=ú?hn'D–Ëõ?t½±¼Ôà?b¶\eŒé?l²…µô0?Y'¯Lå³AGN4FGL J1127.6-4920?ï›wÃc @&Mv«XÀ:^ȋ­À<K€\±±¾@
P_=þ@@6m
J?Â_ý–™4?ÀÚÙÕÉˑ?úZë=Ñç@p
«T­¿å´d@q_>?ïû2¦Ey‡¿ç€"Töοâ¢+¾Ê«Š¿åÃà‡ÿå+OnÓrAGNbcuMRC 1125-490?ï™ï»lÛ©?zÿɳđ`?[¥S¼‹¦-?Q¸å?†f¡àë?y¥É¯â2q?ï{Mï‹?"æžÔÏ?e˜I]ÌÂ?qÝf‹š?‹Æ‰Êk4?'Ñ8òXÛ5?ï	ìŸ>ãÚ?†Å¯uÍ?tÍ-§yrZ?s‹ØNѲ?™ ©I¹'?'NmûHô°?ïñ-Š—?q<.5Ð?‡gƃ"-?erb¿íà?'nS:|¸?gŸ"ÎþL?îÜyÐµå?'ˍŸŸÉÞ?}½O?u›£z''?hDhãå?ñŠBú֔?Ù×ç?©>¹DÌç?ôv9?±Ö"S?£2ü<4€?¦LJµŸ£c?í¦m–Ë!ì?˜÷wÆ5.
?‡Ø¡:Þß?}ëÙ\b?¯£%,¶÷‹?–k_¸~5?íÃñåòû?~0Gö'¶?œê&'ô‰?ƒ,~LÜޅ?¥KÎ\/[?ƒHÔ	v9AGN4FGL J1127.8+3618¿ÓˆAºÏ8@Qƒk¹Œ~(À9m©PÇÀ<!gÝ^ëH@PÚqÐý´@в\Þþ(?¥·ÿʧÑ?¥õØ£‰vP?þ­üwµCC@侬ùrÈ?ë^Ɣ¤gS¿å®É¬†Ü(¿åøq–EQC¿â=fȋõl¿è"‹BhÛ6¿ïÿü¥¬¨AGNfsrq3FGL J1127.8+3618MG2 J112758+3620?ïõrQ{º?BèÈ]7?3Ri%FU?&QÊG.H?PFÃ=-S­?@F ‹f×?ï˄ԡ¾'?v>Iº}È?KM¬ñÌB?X%UXÜò?vÓà1ŠP?rÐp±F1?ﯹnÔ§•?}FÀÔ}
?[Ïgîé¸?g¯g­Ï?€—·J9I?y'ÕÀ']	?ïçaF¨E?M"¾"èå?W>1D—ÈØ?A¤kU^c?YÿAÐð?AãŠwòn?ïí|•QáI?SMãkRg	?@%Dz8¡(?4^³øý«A?\ô3$æÛi?QŒvç¯?ï{3Óþ*¤?ŒþqÁ€–Ó?X9ì,èR?f-"i¼?Ž+Íy û?‹š•>¬hG?ïC¿ÈWr?'ªÜÞÏñ?c—|º
j?hâÌó¡ƒ?‹I0讔M?€é.ÖwÞm?ﺆ'Ý–&?mƒcð:ö+?qLžeNJ7?aXª˜DÜà?qpÍŽr?a}Ì(I	³AGN4FGL J1128.0+5924¿ïÏVûöl@KU¬îàóËÀ9æ±iÀ<–[žŒG¡@ÎPV"œ@T¤°N?´ŸÈêTó?¶r:@SéG?ÿþÊuÚx@ªÂ»{싿ÒÐǘ°eŽ¿å¤ "ˆÞ`¿ä¤{(߿傚Nʓ¿ï¸Ê·H׿ïÿÿ" 5•AGNfsrq3FGL J1128.0+5921TXS 1125+596?ïóÊ'+'?K£ÞÁNuˆ?BÆm¼e/?7#DåBÌ?NöåÃåË?D	Ëýh‹?ïÄfÎãtÑ?;$Aöi?Y+@¸W?p
¹  ?wÈ'a‰5?röú×yßw?ï´È‰œ ˆ?wéYÝÛT²?c+^©‰Ì?mÁ쇜Ô?|¥"ª»R?pرÙí¡Í?ïä8œ²0r?Nm½øà¨w?\M_Ÿïý?BTàk˜?[Af¯ì—?CŽˆrg@?ïåç¡ Š`?]7yՋ7®?T¹ó"ê?GbªjHÍÚ?_w£ ë*Û?VÍ)v€,?ïVšûæ¸(?ž'½õs¨ý?dA,+À?Ñ?z/.¡Ò?'¤zõÉÙ?›×µæ	?ïqƒlubò?" Ãùà?k*}äW'?qI‰GÒ%¡?ŒÔ£5Ǚ?'ê4¡{E?ï©õÐôq?q£CÈ?vã^Ýњ?f:L¨?t²!+û?c¨–+ÿôAGN4FGL J1128.8+3757?ïWŸ·üí7@Qd~¡ÆÀ9ψ*ÜLÀ<	óˆù8f@ÂQ} <6@?f"‹?¼ÚeÐÝ©?¼Fí¥4'i@£ÂÀ®@½Œ¾)q?©×•	'ú¿×®sûû8›¿åì§]§{¿á'Á(SÜ ¿ê²œÕŽ<n¿ã_gÍAGNbll3FGL J1129.0+3758NVSS J112903+375655?î¬Ûæδ6?"•X$L?…ê[(ϊ?xV½t¿Ãn?ŸoU"Ô_s?_@_õ?í¹|Ïùð?®8n«`>Ð? ÓjR?¡ægÙ|4c?¤a_"Ô×µ?Ÿ×ïâóÍ?í$ऴÅ? í# ÄÛ7?ž)'ï3]?"Ù¿¾5I'?®£8ü6L?˜O€›4?ë"/)ä*?–Ì_$äÍ?µúP*\Al?"/x°jì?±Œž^kA?ˆ+žÜ}°?ìò\×zƒ?§Ug§¹Tæ?ŸZí¿êì?oW
YÉk?°–]ÓÇr-?¢]ç¹M™/?êá¯Fæ?ÁŠöUåÃ?µ~þðãW?¹{UùI<?¹Éø²ñø?³—ãQ—¤?ê…öÈÁ?ªØ~æø¸‡?­¶8/Î"-? Ùc€z[2?¼ü3À‰?£a[&ѬÚ?äAôKcM$?¨j¦Õ·"?ʌÁàƺö?©Oqÿ¸¿?Äklñ¬{? ´Î'ði&AGN4FGL J1129.1+3703¿Þއ¨^,@Q€Ÿ¸fäÀ:<‹FðYÀ<`'o@á'C'¥.@ðäFfß?¿*^x[[p?´1 ‰Š?ö¾aßîé@"§×Êת¿ï ˆ!ö?âCbn_.¿ä›ª€qªg¿Þ³æ¡à¿æÔÎùÍ·¿çÁšÕü4AGNbll3FGL J1129.0+3705CRATES J112916+370317?ïõÉük~‡?>š;¡nœG?0PʍmŒ§?&q‹ôJ^?PWÔ&Ešõ?8·%R6‡2?ïÛüxa?oÆÁQºÎñ?CÔ$·ÛbÉ?M"^+ r?oó¾ù,?jNyÆќQ?ïƒïd?eç¼cßRª?R'Ÿß.PW?Pãwp?xà]™×?c®æÉ×[½?ïÀÉ.Î{?YóñŠ?c£ ¼6?DI֊ÌR?vi{B?V«\øo'?ïï͸…,?HB¾ÙIÌ
?8­+8U³á?(~Ðã2'?Z9D&x?Eô¢±æ?k¡8Ê?…–Î|éúI?SE§Á?^‡‡d‹	|?‡(°=îú©?ƒžôeS;?ï¤	"Ô7û?r¥ôh>¥$?]ôŒáz°Ø?d[±w ç<?ƒ?	&+¥+?mÖìDér?ïX*ٝj´?vq@²ì1²?y*ˆjvY?a2kû
S¿?l4G	Æ?s¹7C	&\AGN4FGL J1129.2-1014¿ÔâÚÓÿ#À@GÑn¬†hÀ;9ÌýpÀ<¬Ök±ÿÂ@âŒXhvâ?ý²—a°õ?×5E2E?ÊQÈà5j?ò=0ýÎÍX@ÍîµÕº\¿ïâЯ°\T?ïgÂâ=Lg?éííÿL{Ú¿ÓVŒúk¿æ'4JŠgÍ¿ë#à¯Ø @AGNbcuNVSS J112912-101349?ïØÃÝSÇl?]òjÏÚY?L9ˆJ@{?<i"×´=?pàdTÎn?YóÚÎZP
?ïÀ¤

ðÊ?{æ`3&â?TñyÆDe?_ús½#¦?zqœµåÍø?vYb¦Ï?ïm¯àÍÖ?}rFž;ì?kÏÑãܹ¢?j='ö¡¨Î? 'Õ*?xUd3!ê²?ïV?–‡°?±{]zvÂ?w§vkp?e Š¶î£?—"N2i?{³öÔh£?ï¹m2ø¼?n'2W-?[†ýl3o?K'.o@?|g§\7|Ü?kÕécz´?ï éXy•?‹rm
}?j¨½h˯b?|Sü4!"m?˜½;‹ü‹?™Sý§6ðj?îûÅïÊ?‰–öþ®Ú?v,\¹Æ3 ?tÍeºù'?šü*ܘ3ø?…1dp€?î\äêGSs?"ÄYñý.?wû	Òx.?t3æ™u+?§2P6ޕJ?"§Mî<·€AGN4FGL J1129.2-0529¿´Ô!J•‰ñ@IçiüóÜÀ9¢š4Ê(À<$Sœ_G@;°É6@ÆX>…w?¶¦¢@²!Ñ?½2XíW\@sbb˧3@c¯˜	?ïzÇw"¿èhǍè¿ç"F{åS¬¿çhÁ?O÷¿ïÿülò¿ï³½œ®!AGNbcu2FGL J1129.0-0532NVSS J112914-052856?ïíq5Tÿ?{
O¾0p?LeҎv?a.Û@s.Á?Vê¬AIö?r 7J€?ï'Lj?T)?‰§è–ö´Ï?l4¯;ĵ¨?y̝AŒÄÌ?"@ò!9Èc?~õCÀ÷dý?ï
¥S×?ƒ¤Õy§r?u *í;o©?~lìûQ¬?mA7s?w"'m;E?ï0]…?sü&Œõ²?‰Ü»®÷Œ¯?l<ìŽ2?Šž"õ?ešÇCï™?ïÞ·W¼÷º?e¨v (&?^èµ~"?XÛR¨l»Ø?b3¿
´+?\÷e¦\
?îÙvGò;? ÌZ½	#?~§~VªN?5p(¸?'\£4œ?–ÿøÇr2?ïMêf­¸?‡­¯ZØ?€·ittk?ƒf.t'è?‹Íüݼ·?}zr`'`?íZ.%=e?•îèÜ,w?§¬Ã7º¼?²ß›>?£Epëƒ#ê?‡ú7´ºAAGN4FGL J1129.5+3034¿çzcªŸP@Qð¼¾aÏÿÀ:¾ƒ""^ŸÀ<•È¥i±@«*"ýM@<§P;¶?Åׄᦣ˜?²Lêi?ë̘"¶ÛÊ@íØ>šð\¿Ý"±ð)É¿ç©¿+¤t¿ä£TY©¿âÅõåÊË¿ëýØ"kdÓ¿ïó ‰ƒœAGNbcu87GB 112657.9+305242?ïu—Ûè?·¼¸÷f?lÛ»X­?'¸Æ‡B¼Ú?‹µÒÏ	+ç?²ì=²;q³?ïÓÄ ¤?rh‡©3Ã?HT¬u\?QüteC¯å?sZÍñWù?n£f^1?ïÅ…ŽRq?ˆ5®Et¿ ?^ó]«¼ç¾?bÀºþس?‹°2ò¢r§?‡¬,ábð‹?ï¹%ÒÛR?\.œ…
CÖ?euíE$æ¬?FïBÛ'=?x² ;CSæ?Y*÷¼ÅÜ®?îÑÙöù=?¬Ж´L?wÇÖh	M?'†³Ž'k‹?ŸÒˆª^?¨×Éä'ÄÌ?ïðª° ?‹Ÿøà$c?XµÍ8£Ñ©?bŽ
÷­.£?ŒmA¯ŸUË?‰70BèÝÏ?ï*q}ƪI?AñÏ×v?hGYyѤ¹?kTì)–?—¨å8´N? 䉼^?ï,ÁD‹þ¯?~ÓЦî?~]ë@FìI?g|p2©à¹?'Ð\¥ý"?y3Xƒ AGN4FGL J1129.8-1447?Ò¾P³ Ô6@Eє[l7aÀ9qÈÉ2
™À<ë˜iî±@,ZÝFA®@<bÿ©˜ë?²ýáÛ¹¥?ºWA°N'Þ@ƒ¶æ±za@
'õèO	¿Øƒ´?3°¿æ'Ž¿éŠ¼‡k ¿é+'Ëöä¿îC+κ㖿ï°ÿ|L¹AGNfsrq3FGL J1129.9-1446PKS 1127-14?ïô#Pŝâ?F¾Ý—;˜¢?6Èє‡¢?)[œL&Ÿ?R*P<±?C»\æà?ïßo'ªûÓ?l~qS¹k??m·:n?EÑÙlâ×?l¢ÆW{0?i%Fk3R?禍娀?wÂÙrbë?d©ÍÉz?i¬'Óý<?€q£¡¡x?s&
rŒ–?ïùÒs¢0Ž?-ΫÆDœO?(P2ºØ?ô+¥á¾?B¢
o/™w?)pñ	±+?ïí©Ýù3Í?UØZƒ?>BˍÎ?1h)½9ñ?]Àž4{?SùÑñ"|#?ïš÷3—uí?Š
9,$(Ý?R|²jºK?cÜsŸé ·?†ÿãƒ%AŒ?ˆ/֞­Œ?ïeÀ^Ýä€?…|Ä÷–O?p
Ä|`Á"?qÿÁô.!?ŽŠ†
®uB?'zž§?ïî)§ ôJ?PKW&X­¯?Dq
­5¦?7å`W'û?Yt)ñ²x?JO"úRúAGN4FGL J1129.8-4217¿Ð4r•k.@2˜ú7iÀ:Ç—×øzÀ<¯¦âWx@Å°ù³@"`št‹?ÉGHÿMR™?á|â(ԋ@öOv_Ù@'·þ¯¿î l¼Á¼Î?îPz×6³¿Ù·]d_%*¿ãä±i¿ð¿ïpêÄ.™AGNbll3FGL J1129.4-4215LEDA 566417?èùj%ÒfY?"ðj6?ƐªÌ`°?ÁgãR³	?¦&²tÆvS?©VÞaŒ?ë.âG©€?¾~u¯b6_?¸¾ºd":ÿ?¸9ýh"?Í?«"fÂÁV?£âŠ>Ö×?äSÅ`-#?¶$î'ξ?Ò! òf?³È1(3SS?¶ÈÞj[P?¢Ýc¸€m?ì™ÕŠÕÃ??^«*<t?²9læMËg?Š\-T+cL?¡ïÖGq
?}W»ˆл?㦽x¾O(?È	Dcÿ{B?Ô:N1n?ÉIŠmVŊ?±áÏ%,?®‰¼Û&Ó?æ̏øRƒþ?ɱBI`Ø?Æ}	7ƒœO?ÄJúº›ÇÇ?¼¡mÎd§t?µê¬¯^?Ý×å}%x=?¶cþW?ۀœU"9¼?¶ÔÍV/mž?ºø¹d»?£øÚt"A?èe½n,zÕ?¤ð.¤ù·?õÝ…ÿ<?¡ÌÄ_(€?µfZƒØ\æ?"§¥©AGN4FGL J1130.5-7801¿ïXØy(_ñÀ/¨'ÿ'À9ÿ_,¶ApÀ<…I€|'@!Gø%ÁÃ?öŒ©[®|€?¾ ﹶÅy?ÅÀµ§Â&V@	‹)CÆ(n@RҵſÈp¬æR"Ý¿ïÿíáoq'?ïÿo¾ÁÇ¿˜ìû7昝¿Õ‰ yݒ¿ØÈ\ûƒ™}AGNbll3FGL J1130.7-7800SUMSS J113032-780105?îçE½Š ¿?¤*c·M$?lP
4Ytv?f•ãîݱâ?ŸG5¤?£¯ÿx§¤?ïºRaKÊY?'?õ\7·E?T€Ew½Ø'?dYX˜"ÑV?}¶¾ØÉR?€Š"Ò¸/?쥫£?¦>šßãØ?t'½XðÄê?xgR"‹^Œ?¹‰‹…^î?¥î!–‰¶ü?욲tm {?œþî*çö?fªgÈ}?UõɲôY
?ºu$Ǿ#?œòèÊp?íÀ†ÊMÛD?®¶=DRA ?‹7Õßdë?ˆKV$3ó?­)ãIHÆ?«¯ƒûG•ˆ?ïMѺGd?™I ÎeTù?h³ÅÍÓª±?|f
®TE¸?"/OöMÔ¾?•³¾<nÏ?êqs?©¢,àê®8?Ž-G–)"?ŠÏ2¹­ä"?ÂanšgtÙ?¨Ô{D+ï?é Þ>[¨?³-¤Ï%ï2?uh[úÍÊ?rG'v±v&?ËFÙD÷£2?³fÛaë ƒAGN4FGL J1130.5-3137?葽í@@<+-À;œ%¸÷,óÀ<ÆiH˜ö@#ÌP×H?õ~z#²Œ°?ѓa^j?µ|ã«`–n?Þ¢èB2›@e‹-m?ïךÈÙ"¿ítÎ6/g¿ïù–#?ïïšø>jŸ¿Ü®_¤U_¿=aƼàAGNbllNVSS J113046-313805?ï!kAÇv?¢»(F?A"i……½X?<>熓2¤?›EóJ¤@?¢Œ¬Uœ?ï"Nà jr?ŽL¡}Å{ë?aMóq??qfÛB¹ì?†™.kù"?‰Ï°§´+Å?ì¶Ë¿Â´V?¨-"KrÕ?YכH¢†?^hR1ú›·?¹å:¤8%ƒ?¨9vco?ï!-*Ýé?†DÍêµê?^ŸÐ'eë?W߯ê:ì?™ð_û'£?…ȁ˜/²?ïAÿÕÉÜ¿?š˜e}qì?Cy+Mì?B©)Ö=×E?—$;æ¹q¡?šDMò-,Õ?îØ&AÞÕ?®²¼ ò¸Ì?llÿ@í"?";êµí—†? ¶Ëñ•
?¬ìö=-?íDÁ¾%êö?£[Æ,þ?`÷º;­Ê?i/ˆ¼y-î?µR4=§Þß?£žwn"??ìÖtêžÖ?ªh$5ý-Œ?€ÖÊ üP$?†Ì‹52#Ú?·1WЫ¼?©5cuVzAGN4FGL J1130.8+1016?éôBö'l´@P'»ƒÏ,ùÀ:e$Ã-çšÀ<b(Cëè@áðusu@Ëeè'?ÀÏa<0?¨?ž)\?âùâå=@s¦¸»ó·¿¾Ä(cvq÷¿çË@Fìù¿é%ØÝv¿èO‡A¨@ü¿ïâöý»'¿å§/^½O¬AGNbll3FGL J1132.8+10152MASS J11303636+1018245?ïÄ'EO{¤?pþF9?c<j…­?TŽ[l÷ò?tf¿!Ÿ:?l0<‰¾?ï}YYZÒ?Wo½"ò?m¤¢ç—¥?uºc¤ÑAb?‰@€ö {?‰µ´·•?ï1éÚNÀ'?'Þ£§85?zaî֎¡×?udgÆ~M:?"*H÷íAI?},ãÞ@M‡?ïXn'›°?sWçßÙ-?†ÀsŸ…¹?m©"XÓ?ƒ#ÜMPDV?cCZÁNk?ïN´XC¤?Š¯‰ùq#6?~—w×E?u¿^¹Z?PžMê`à?"ð½(%IL?î"82eFÅ?¥¦4·¶Þ?€ò~Ýâ'?ŠËŸúç™?¢Ý"2ïf?¢—֍û1¸?îj›–§?'œÿL\T?‡¨_Ò?éÇ)W7?£lCíb?Ÿ‹Uq3?î±òð'?'r;ò¶?¡W'fŽ77?•³µçÍ?›.¦òͱ\??³¤¨°AGN4FGL J1131.0+3815?­¶Æŧ@@Qtw—|À9/ͶígÀ;Û£ûkq@‹D¤bË@d[Ëر?¬yð±ÙVs?ļ3b(¤@Š.Ýc@6c¿B ?íWZYè©¢¿äX·¼šO¢¿ç?³ÖhW¿è܀žöѿꦭj0ö¿ïÿî' ÇAGNfsrq3FGL J1131.4+3819B2 1128+38?ï¨ N:[Ø?~óY§áR?'HÂӃ?|:_;•¨?]yL‰{ØS?U%\áM|{?ïQM`Â?…[eñf?k¸Åúº·?s
üæD?…½{ 1ί?~¶¥,őâ?î²ñùI?™4§¥Áˆ0?"Ú¦g"òö?"¥"L3?"Ç86ãæ?&äÂÎ ~?îâC؃–?Ãx›ãAú?"6'Û†ÆP?xcïÑz)¾?€òíÜü?vØËaÖr]?ïW¯ÿ·…¾?¨Â¸?ó8ª÷?Š=Z–ˆôÚ?p[÷î}½k?mÒ$9˜›?îŽÉž?«;€>w–?‹{ëÜy?¤ý‹7hÙ? 4kY¤½ã?›âwÕ%¼?íô~˜
? —f
¦ä? ÏkªÌ[‰?™!Ábߔ?ŸÑU©œõX?•+¾eOê?뻣š÷?¢FÏ× ?´3îA'$Š?ž&»ÿÀ­?«ÝòßúÍ?•ô ¦S;fAGN4FGL J1131.1-0944¿âˆºÂ;×Ð@H(A*2À:Ò
¨y0À<‹Cp˜@ ;øå¯r@"÷…zÿ?½µj/ž©#¿¨0€Á"Ö?î*käT¨Ï@u<Z#?ïϤMQÂj¿èZԂ"Úv¿â7}DÏ=¿àeòmpEã¿Ù˜,F¯çº¿Öç`Ÿý·AGNbcu1RXS J113104.6-094353?ïÃaûPK?is)§Ãz?RcÁÔtٕ?<$¬!À?yß^s͈?h)·^#•?ï€w3ùÏ?‡²Ð Œ•	?f­û°Jð?i‹›Äâ»?Š6Á%þ.?ƒmw31•'?ï:!±M?rƒÐ3Ó?_\9‰ßøY?E\'÷Ûs1?ŒEðYÂ?pöœŸºû?ï'É"(ß?xÖ´rZï?r5¢²E¯±?V¯`s'×?›@> ±'B?xÞggŒèñ?ï†ëé6~±?zP³g?d;þšÎ?^^>C‰?‰6@,5«?w=Û]¬T?îÁâRðè¶?žOéaû?qìŸ/Œ^?y	°8¯?¡¤Fî<cR?š‰`Š†
®?ï1Ø%"?…R`q›(?iN"†¼'?\à%Kiaû?œò{™Ç?ƒÿŽB.íä?ìz¥DŒj?–Ö|2‡e?6äqë?zþ42À|F?¸CùQî'Î?—è¨AGN4FGL J1131.4+5809¿íϘ4¥à5@Kú¦">jÀ:}mÿ·Û¤À<²bÒ]/†@P1ÏZñ"@M••_?¼´È?œœà²'?âa…V¶K@þ•dU¿û¿ïqsªò‡q?ïõµú"pm¿æÇ1¢a‡¿ÑT‹<߄_¿ãí©¼&Œ¿ä½öp4E'AGNbll3FGL J1131.1+58101RXS J113117.8+580911?ïìl%7i?Råœbç?B[¶òáX?31Iއ?^Ÿf¤Ý?PŒ	 ·y?ïÙJÌv?qæ؁(ç?F)ð8qqH?PÛö®Æ'?p®?®Š?mY¹Ã5f?ï¯Tïú?s{äYà¶Ú?SŒ%TË?<Jir³2Ú?¹?fô1?sF­™áQ?ïÃä'Á»?XGÎRb†?h¬oü?I¥Æ
HÐJ?q·î˜øR˜?S$ƒ†t†4?ïß³PÇ:3?`rºeÏ?Pâƒ?D±< K&@?h=>d=»þ?\
ft¡è?ï'ajd^
?‰c¬¦%hü?XÜÑ3-8Ñ?bò>l³?ŒLIÉÈm?‡bÓQs?ïpM›ûYä?~qÌd"J?\ô6ÐûöP?Re©ÿ4ˆ?'	D´?}µDç+ðä?ï`ñqiF7?uH8ªø°æ?€%d?ÿ?fAbq)?‡B•p\&?oD´Ì».AGN4FGL J1131.4-0504?×"ãøô"@J9Wÿ›V2À:¡›Æš"À<H­œ…Ý$@ˆsü|@¶ð<=ð?Ê-ë˕•(?ãØYÞBÀð@cì‰*¶@	ùBWC¿ìŒòãÕ¨?áœ#íEY¿æòŠêÕ¿êw»ûS¿è«ïxÉ??Æ­°½L§#AGNbcu3FGL J1131.9-0503PKS 1128-047?ïu~'´`+?f	ƒK3?‹Ìâóßô?Ž]²TÿËM?kNL±¹ìå?e†Å³©<[?é´ÐjÖ?É·{ÊÉ	?ÂKtÄ3\_?ÇJ*,¤?«…&Ný?£ƒÂàlÐ?éÂ&1ܶ?­Å(D•üÄ?¹ioÚÁG­?¤dŽÈJÖ?¸†ñŠ)?¥a
¸jT?ê¬Ü»h‡?¢TÌin'?¾¦Kˆ‡3? 
½,?§å?uÉ¡?'îµ(ÓD?ý@]?¦${¿?¢>G£¬?£›%+zÛ}?"Þd»¼¨?‡Í¡dèW°?『ù,§(?ÐÄQ ~?Ñ®A¶ ä?͐¶;eÜ©?½B^(C/?±~ˆN^+?çpuUd?³‡"Š§?ÂQ´ä´Ü&?«'é0v>?Áp‰Eõ"Ò?¬;s'!Ô|?Ü£
Ûj
T?¸Y﵅'?Û,›
¯b?¼7Kr²?Àa±êÅ?ª€EÖÇúAGN4FGL J1132.2-4736?î+"¯ÔÞ@*R¥'ÛçóÀ:&vŠ ØRÀ<K½¹3'Õ@ üSøû?ÿÌð©Jç…?µc+Ì¿J5ÖD¨x?–Ló½kI¿@"NÀ,€g?ïÿò(¦è7¿æ{B`Í 1¿ÞžáIå¿Þˆ£Ós¿ã3ªò‡qy¿ßÝ~ ÄÜAGNbcu3FGL J1132.0-4736SUMSS J113209-473856?c6õÏ?ƒÊÕ{Ç÷{?M¯€,³4?CIWo"}9?‡¿¬Ccƒ½?ƒ<|´Û?ïQ†)8†?œâzóŒ
W?VԜÇɅ?cgôßÿA?"añ"̳?›hc¢®ï?î‹ŽFþ?—ÁìdÏü?hÍZÅ('¹?fr2î°õp?¥Â1l£[(?—ŸAÍµ?ï@³R8˜3?pƒx^ GÏ?q•¡2ÜH…?O;ª²ß?""-n°x?müe'3Tz?ï>ð6©?"ƒV·à†?_·{Üä)Ý?WŠ.:"­(?–&€ˆH?"ßÅàºäo?sz?¶"¯‰±IX?dCmÃrö?qGÞ?®yþ\‡'z?µþ‰Æ¡~?íM»dù?¡íÜQz$?uÅ¥þº*?mdæE,!¢?´A؄Qc?¡ŸN`÷kÑ?îè]]9}?‰#´vOù¤?‡Žz[ç?i~«[œ·?©Ïֈá†/?ˆ
Á'Ãs›AGN4FGL J1132.7+0034?íזr{P6@Lµb8Ú<!À8j¬=áÀ;ÎpmP@–Eý`@åM|Š•?ž±ç÷©"?™­ƒþŸ$??÷¹÷2ú(@	á þ'bÅ¿Ñ:b|vóý¿áX»]c³Y¿â¨B(ïb¿àíàBËV«¿ãÜU•:¿æµ£ñpwAGNbll3FGL J1132.7+0034PKS B1130+008?ïë}1âƒÌ?g͊þDjÈ?5ÖXvq?+ö.}áŒV?aß³x¢±ü?g‹O‰•?ïm +"s?"F»­?oÖÖvÓÌ?|øý'?Œòÿ"ßÆ[?Ž:`˜q&?ï'LiBÂP?†."Sò-u?cv"Š¡?t*ͪ¶?†ènS´?ƒžûRÑ?ïwÂl º‹?sºœnl6?~
"9vÏÛ?hKfÜ\$­?ƒ›hÔeU?e¬,¸' Ä?ïÔ¯	Bsî?l! 㯥?E^YÔ_Cý?;M_Z`?rü°	Ÿ?jÄÜô¦EP?î‰UÖÓ
?¬ÕúZ?€Ÿ´ó]¡n?"ÛGüÓV¨?£BµS«Æ?¨4Kê—Â?ïV1ÖÍè½?u£þÉàc?j`	oàK¦?u:máó6+?'íÃ÷Âíñ?ŠŒé,àÐé?îé)^ôD?‰S_w:Ž?æ62õ~?×ÖµÀ¬?'ÑíëLáý?|­ÊaAGN4FGL J1133.8-2048¿ïòIÔ4u(@CA3 @|ÈÀ;J¥»æË|À<¬.î*§@ #áÜ~q?묔é0°¢?ä#²VÿÁ?í'I†\@¥#±µð?úÚ!nºË¿ë<…ÂL@?ïèq£±J¿æ­—}_§?ËHvü¶Ÿd¿çù_!£"ÿïúDÕ&§AGNbllNVSS J113350-204852?ï5Í
S>…?™:ËÕl]À?në]"áä?nÓiŽd?•hò¤üü?—6jH"Ú¢?î' šs?ª@^+Œé?"¢—R"
? êúíîñÀ?šàä¢O¢?™Ò6éت?íkI×Üu?¤A"w€F
?"ñQ"$óE?"¹ϼÙI?®ÒÅD¤<
? EK¨Fœ?êï=Sâ?¨[ô}­å2?ž_ß:lö>?–Û2w=҈?Á¾Zá*°?¨d=nÚÛ?ïägÚ@?—oŽ'Ñë?{M`ì	/?yšd'ñXl?•0ʽ›/?"K*?ìm£ü–`w?»ãƗIú?¦Ý݉y?±¥ya
˜?±…q+é'?°•V
ÇÖ?ìw8kVe<?¦™b«àˆ?˜{â/§»Û?"+Ö&û‡ï?¶'D>Î%?£"ìêü%?è#'/±¸8?¹ÏЕâ³r?œx¼òg¥¦?¦†¾;2²º?Ë⟣Zê?º3ô8ÌzBAGN4FGL J1134.8-1729¿Âùéæě@DÔ€À;Wc$'†À<¢Y …F%@" Ӊ)‰ç?ôÁjî‹?ä),~ä®?ӂݕqì¬?üýî'ð2-?úkQ'n×ú¿ïƒŸâˆö´¿ëÓÂõ³uä?ïúgïÓb¿åfc á¡ñ?¬Dà"º^¿ÛUü wnÌAGNbll1RXS J113443.6-172853?ï®|­_?§dþ¥jË?\ñ!KB^J?TC"ýx?œ»U~Ø:?§Dÿ%žüÙ?ï]
Ô^*r?'ñA
?mF†¢Ü(?r@¡Mʐ–?µÔ¬¢ÝQ?kµ¹=s?íi×`¾J˜?¡YÈ*Hv?8—ˆQY?~Å«òìÙù?²ŠC†lµ? ñüó`S`?ìµ[ö­¡?hûmÔVÊ?RÃƇoÏ?Nu%Ii³?º
2Ï­t?Hù(©Ù?îK–Á?¦º/L"ú?oþ™áX™ ?gçVBÜ8?©N-Ä4á?¥[cy³0€?îTMlì¯?©h^ÜUí"?|M¨/V«?Ücopc0?¦\Øîéä?¤™ãMd.J?ëÇ¢Y9_Ñ?¬±ß=k/?"µ èë¬Û?'–Šë0Þ?¿,Iãd?«òëµê3ð?èg1x¯$?´­—g.U?Nä×ÕUúF?]"•}è—?ÎDUF¥Î(?´ššQ°çAGN4FGL J1135.1+3014¿ïþSmwí@R@I<‰ô
À:ŒNrSÚsÀ<^6=@IϚ¦ã@ôQƜ1$?¿7)!Œlµ?†æՕ%õ?ËoY­€@_²ïyu?¼˜-žHÕÝ¿ä©Xž§ m¿æü­e(¿ß¦+xSδ¿àï€ô‡&¿ïø
ÞpAGNbllCRATES J113514+301001?ï¯Á‰Ö5µ?°÷s-bþl??ÂFϟ4Þ?UÈBå²ë³?ƒ‹`£[H?°çÿ7(g?ïà–ÿ§ã?p"¬5Ÿ<z?:zó}ÝÑ?F‡oóõZ?l¢¬ÆË?nPäXÍ~?ïY<¦hMá?ï':(¥?Tp'í´O?aQÀÿœ}Y?"'b™µž?ÇÒùÓ?ïè‰<ôï?DÇhšC·?BËko+S?'HAG¡4%?bÃéMZ׊?B"BW(¬"?ï«Då^³?9'É/¥?MH{ëòûŠ?L~áò',|?ƒZ>ô2E?JU‹82?ï¡&+kqF?ˆLÒ6[@I?N"fö›½g?Y€¾"-[?…Î.¯gwŽ?‡!0Ù?T©È?™ä6Þ©è?^ 7àšs¯?føu-dÎG?¢ßŏ +à?™¼BÒ<Â6?ï¶:‡˜î¬?g§Ó5u}?^…-n}­?J
ÍAMf?}ApÓʄ?dß՗9€ŸAGN4FGL J1135.7-0427?ï–Ã`E@JÀI¡3ÁÎÀ:Júì.'À<'cXK@4¥šõÿ@´£@ˆÊ?Êóˆù8e¢?ւc€Wÿ@<»r1v@p8²N¿âÉäà"Õ»¿ã²['ÕÝ¿çéüÞbvm¿êTÅ¿'Q§¿ß^?cR¿ïÿ‹Á>ÏAGNfsrqPMN J1135-0428?ïêJ {ú¼?[š]ÇÚíE?Hy°}¹ú?Aúë?_-æ¿P†*?UɅÛyËa?ï¦بÎ?ƒý‰W&t?bŒÅvpb|?jº¦øyí?ØÇrÀõÓ?~€ñ´èy?íìGVß=p?	ëD°T?e©wêª?‡î¿0š5?©b 4¥P?™;Qyj0=?ï<Hvß?t,çÄfÎ?w4~ÓíÃ?^™{¸o_?'¾Ò³ø‡¿?qÌ2n¢U?ïÛV.y©Ô?kÎ59iz?R	ÍO{ر?LsjÈÛ-?k¤êût÷—?g¢
^¾{?î×tId3B?¡ -¬gzÙ?z²–¢¼«‰?†»)DŸ?ždÑ0¡Âå?œ¬p'MH?ìw[ò	?¦AøP'Æo?˜2e»˜2l?éµ•íu`?¶6ã¯Ñå?£ß
·Êú=?íJW²Ìù÷?–ºzSœùå?"Ö*–N?'I9Aƒš·?°w·Än6?"–TÐÙ0AGN4FGL J1136.0-6824?çU;ù!áÊÀ3wÀ*ýÛÀ9ßzR÷À;Ý=ïí™@À¤[>•@7Á•aü?ÁÜæujeO?Æ9,œk@þ|Tå5@;BÄÕ?ïó˜H`Áâ¿Ð'¿ŒÈP¿åú!ßxËï¿èûYbFò¿Úa3ÁÎl	¿ðAGNbcu3FGL J1136.6-6826PKS 1133-681?ìÛ.ä¼O?¬Åó¨çg?
©'.ï?…l®3l"‡?µ#ÞvÃUÖ?ª¥«§Œl"?è1¨MUb!?¾"9ÙüœY?ˆóN#-ê?ˆFÜs¸þG?ͪ-æm1Ý?½M²‡É"æ?ì\ËS꧘?¡?/—|›Í?–õ–Ó=?¬?Š~Sk½?·\?ª'˜×?œ†{—–ƒ;?ìpÿO3¢?‰ŠV"\)&?™)ÃDy1?y,¼¦Uëø?µC-"µD ?†ã	
{ë?çn™}êçj?¼AµEáO€?§èAÚ§?¡LEôn?ÌK™·Ý¸"?»]Àƒž?ßÙôÈ¿L?ÈüàÂ3Qø?Ÿ¬ªc-†R? ¢"Én?Þ+@hîV?Èwwù¿QÃ?åËó,H?°ÏрÑü«?±±°€±? zÂs@?Э;¯P?®!i2þÂÚ?æëVØ _h?¢…þüݧ4?°¡y_Åëæ?™)8•n?Ìç­? ¾xÊaЏAGN4FGL J1136.2+3407¿ì˜Ä"Ò–@Rûüe@ÌÀ9犰ȊHÀ<}Mæ<à@¿8Ëùh6@ÝGËÂâ?µs[|T?¾w¾}~°à@.¾`"€@Ó×½k°Ó?ÖùXD¿ä´Ò9ô"¿æ{{*·å¿é%ãõ~z¿ç`…¡j€¿ïÿû}º@AGNfsrq3FGL J1136.4+3405MG2 J113627+3408?ïù‡aÍiD?D24:ŸŠ?/@H²Gý?1ÓÑÀ¯–?BgK.g?A­>mÆr?ïá#‰î?káÎûù?=DMñ6âo?GS¯}‹Ì"?k3í5¬˜ý?hR¬'ËU?ï´Ã§Æ>O?vuAg׿??_{àIPG?iŸšá¬{ž?}¿;:Mä¦?rטÑ#õ?ïõ äo3r?5ïæv=Kº??>Oð?%~)ÑÔ^?IûΌ,2ë?1ˆ åëê?ïõk¤5K^?GؼŸL?;jõÆj•?6Á¼·¤œ*?L›ó˜=ûð?AeT(-i?Ê
™?…ã+Zx?S]!+éNÎ?bÃð=æþ?†m©ediÔ?ƒÄž3?ïyڐ@Ì?–>ò4_‹?iM·àUçz?lµ`Ó·!?‹5íìÝD?~Í,™?ïÞ¢"î?[îÞ7è?ZgùÄh®w?J(hO°?d)oÂ0Ï?SƒCणAGN4FGL J1136.3-0501?ì4¯ÙÄM@J‰¡ÎòAÀ:…0íÕ·À<³çcQ@Íe+'öê@º=c7ݽ?і]çM?Ýî~ƒÄ~@r+EþçÒ@'rÒZ€?ã'ZS<=¿âқ®FÏÈ¿æ̀÷Œ>¿é¦zÞB•ý¿ïÿÝe¡D‰?ïþXËs0yAGNbcuNVSS J113607-050156?î2Ô¥MÕ?´ø\OҟK?¡8²i˜L?²ÞIþ†?—¤ùêª<Ü?›ÿw€º?ë˜ÌþS‹ ?ÁŒSÏ¥?µÁ³<Ë?¿hõ6ù;k?ªñ¶álÜ?¢d^.¡‹?鑙|à±?­²Ôrm¼?²^5FÊ?¡òIïCa'?ÀŠhsw?§¥('¦½?é<Ö¾àà?¤£¬"‰i•?»&†žâ{,?›¢ý˜"?ºòÃpF}Ø?™Š-LÀs?ëfÇKó7?¶€8u,÷?¶eõã}…•?°æé5Kò?¬Ò×ÀÖ%d?§c°cš?âù£¾ûAÄ?ÎWœ<>Ó-?Ñ`sµPÑ¡?ÌÀäb?ÁX‰™qU®?¶;)·Ê?æ#—r*k?´;5gï<3?¹$Hú8Îz?¥­_Á~Ž?Êß}º§–?±&GºW=ú?ÜÝvJ{?³[ò£ñÃD?Ñ.´Ÿj¥!?³õ­Ÿ:Ý?Ñô/êJÙe?¯þ}a>°AGN4FGL J1136.4+6736?­p]úmU@Gú">iƒÀ9ÊÛ-¸ŸïÀ<Td«{Cm@ o@)»»?ûB%YUÜ«?¯bJßž? –´6þÄÂ?óišÐ@
"M'ëð?îŇ^-³?ÉO[¹¢¿áµR\Ä&¿Ô.ÁÙ©ª¿Ø1tí¿Ù«¨$v×ÎAGNbll3FGL J1136.6+6736RX J1136.5+6737?ïï¹êO*?M܃?Ëè ?0éØf'Ÿ? ß)ÐAÏ?\‹°áS~m?K_Rß°ùz?ïÞM~@«I?o^¥\…cð?B̏K?L‡º]"î?lÿ]Š¡"?iÙokGt§?ï´.3!É?u˜¦§¹ŠØ?P4|6?75!lÓàW?€ò쪎b?u]&`a˔?里ÿ1<Ó?]ꩺJªx?cfž·g9?C~,ƒ3µ?;ØwÀ Ø?[X­…ÿœÏ?ïá
ó_Cî?cîAÂZ?@M$ˆf?2ÌlÁÑS?jáÃeƒ/$?bvËf*äS?ï'gúmÍl?Þmv5?TúÝvm¼?`O9÷ç
†?‰¿æ'i?‹¸Š—š§?ïq÷ª#³?"s.4––¢?V"°b'(-?Tß\ÅöhU?WϾ§l¬?"*Ýd¤¹@?ï)¼><Ú?yÞóµ€À.?vä€ukÉö?`øGù¸™?•$èYՐ>?wGP®é–îAGN4FGL J1136.4+7009?ïùi$©$@FÒ·`,'À9¿¤EÀ<	?öå@x{‡µÁm?üÕýb–Î
?¢cŽ"u©X?yÁ"KùÕ?؛Øc-÷µ@
Ãsٖ‰Å?¤A_r>¿ØªÀ2Š—¿ÝžN¿Öš+¿Ù¦_$Ӟù¿à=At>–>¿ÁÃõãœrAGNbll3FGL J1136.6+7009Mkn 180?ï÷
Bϐ?Fù.ë&q?&Gÿ…Ôg?!ç¬r|5™?NDõb´¼?D+ì!†ò ?ïÕz6²?r&µ2¸…?Gh Kú»?Ryzˆèây?r"U—萷?nE"è7"õ?ÒñÆ?K˜.b?Via/ªC‰?auHé•:Ó?"Êß6ܵù?Đk9?ïÄ;gÎà?\ôdœ†æ¾?Y4)$«ùË?<ëa±12³?w•A»w=?Xæ
?—)?ïïXáÔ¬ü?Wó)BÒ?6Þ¼e'Úö?<̨—ê¿?[–Œæ¯)T?Táô'?ï~ÅÊ=ë?={áwÔ£?X[î5xÂê?dε¯u¶?C¢žö²?c ræL?ï\ØR^i?‰g<‰¥%?]Níã¹#?fP=iöÉ`?'Ø=A ?ˆ§æؾW?ï€Óö~Õ?t•ì¬·<?jéߊp-#?TîÝM5ƒi?‰ÁždgZ?qØÄ~&ýíAGN4FGL J1136.8+2550?ë é±¬WY@RQõ@‰]À:¯Q=à5_À<–/#ÙùÜ@ ;%Öÿ*Ã?ÿÇP ©Ã³?ºf¨UŸß¿£Ù,"=Š?êTø³¥@oZN€?ïôÜJ婭
å¿×Fb$S¿ã)ªžNµ¿Ü­ž^Ok£¿±!`ÍË$AGNbll3FGL J1136.9+2551RX J1136.8+2551?ïØZbT¼x?n°Z‹?M¯GhÝüÑ??‰,Š¼ª?pæ©j?k"çô쉪?ïËÂÏP"I?tÈàŒý¾Ú?F*õXš?Jƒ¤
ò0Ä?wY9ƒvn?sn†÷"²?ïyTàW@?yñô§ñÆã?aÇÝþd&?\ê17¶ŸÂ?g•ô/?xoü¤Å3‰?ï'ÃÃ}‡"?jÛ;Š¸?j¶=ýA?QHä^²'?ˆ¡Ÿ¦¹?iÝÞf€ÿ?ï¸Ïhã?oZ²2Ÿ—?\´[1—Q?OÐÚ˜IF?|k(såˎ?k^€¾?ïX¨ÓüÊt?'FmŒET:?[sM2Ù^?bf'æ· ?"3´_ä?'|¿sfâµ?îô?0R¿Q?ˆÁsŒÆu»?jÀHÇOxy?a(ß8V«?ž ãõTÎ?ˆ/ßcÖ?îrU#Ku?‰ãoxNé?ƒ FßÝ~?qez1
@K?¤¨ûÁ"Ñ?ˆùf¡t¯AGN4FGL J1136.8-7413¿êgv±¸À(4¹#¢œxÀ9zŠ‡¿À;ã5ÍAfÓ@Äù·;–@%Қl'q?³z&P Õ?ÊËí>\\!@=s!_Ì@‹ú¶j	ß?ïýaŠ^"3¿Þ
üGä› ¿ã4ýØ"¿æ¦ãÏGÑP¿î:ò¥µ1¿ÑÇÒÝ2¸AGNbcu3FGL J1136.1-7411PKS 1133-739?Ô}¨¸'?Çk=_JØ?Ú¡ý6³+¢?Å;þVü?Ðàï!>Í?ÀEøz?Û)@¬Ù	?ÎÂ[s´?ÛU†ð¶?ËØÛ¨?Ã|ÔØƁ?¿>§Á¶ª]?â²¢)5.?²«M®Ü`?Ð7²ä™G9?°X©¡dï7?ǁϮ(œ×?§ýív7?â‰æöėõ?¢Lܼ(ñ®?Ê\ªñƒ2?ý!9œ¿û?Ë{ºüú?š«3»Ç^?ÃÑ:'•?¸a.‡~™K?á
5›?Åf"sÈN¹?Ó\U8ÛX?ÀáVxúÚ?ÑÆåÒ¾e?Ç¢öBD§?áÎOÙ(%?ËÏÑö­?Å:¦Ï¸¥?À…X«#?×#lÒÐ?´d¥=÷
f?Øàqô}ڐ?µMYòÊ]?ÏøCë^ª¨?¯Ûr%mj?Ò ø6÷¨?£qÒ½=ø?ֳѬc(w?©ŒÁÛ1]~?×6
ZRÿ#?¥f®¤+êMIXED4FGL J1137.9-1708¿è²ÏUh<T@E"_ !¸À:–,Y$^"À<CõwæÁk@ ìç¢fé?õÂFçE?È(éè‹Ð?Ñs}\º@	£qÚ7ï[@)£šyhw?ÓP¯°\S¾¿ÞDÔÛ¹ú¿Îì%'›{?½e)$'"Í¿â6o]…í¿Ô?·¥ôïAGNbllNVSS J113755-171031?ïÓLý£s&?n{sœ-n?UÍ»•.U?O8xKŸ=¦?pæ.ÝäN?h™š^{6ˆ?ïÂR£o?vŸ.ˆÆd?Q·Óq§?V¾è´85?z·x«yL?s.ðV]e|?îçAe%Ç?"~閼Wz?x¿qŸFƒ$?|ø‡z à?œçöùåíW?'åœíÛ?îò'ò1?Œ\mVT&q?p/þ©?X­[0:úå?­š× &ªÓ?‹ÕçA†÷Å?ï™_Lj6½?†4€—vg?dN':î?]ƒ2xšêÖ?""iÊm"Í?ƒçîEµ?ï:øh‡?"‡Ð|X?eÙ‰«%?p -jÆñ4?•åÝP8ã²?'rvöô—?íòŽÒ/&"?ž»nc\‡?‡Jß[̂Æ?ˆ¹"à=ܞ?«[†È1?šÿe²S¨2?ëõQü!#?¦×ò»`ù?Q
֒&?p«BN‡4+?Âå¡Áœ`?¦ýŽRìö‰AGN4FGL J1138.2+4115¿°*ÖVÒÝ@QXŠï²ªãÀ;`OËð.À<±§ðtqÂ@ 4C(ž¯®@,ZÑÝ®?½F‰§357¿¶dù(öC?û{
¢ò)@ÚD…ëçÅ?ëçlU"°L¿èùŠ—ž¿ãù.ŠWw¿åÛWª¿×ÙôhI¿Ý¯çä«:×AGNbll1FGL J1138.0+4109NVSS J113812+411353?ï·E2}ð`?tôºM(‡Ë?P¢-‰ŸM??V¾=WZ½?€m© ¬:?sùak¯ðV?ï•Ê»‹Âý?‡Z°Ð—Ý'?_öTßñÚ?eÃz˺1?†Ž†xÒ1?ƒÝÓ¤'$?ï[€ßŽpq?€ýâ
xR?_÷Ù½îÈ?]–€(>Œ?'gÏn©?€b Çxâƒ?ïW0z5#?w"rFšd?n}5c¥É?X
ã:ÑÒæ?'Xa©$ñ?w'>"h»›?ï1Öq'<Ô?Õðs+W?e4ÆkiÇx?UÖ&Ɲó˜?—™ª<?ŽÂÁ`QT?ïí.éo?œAĵ
À?m)Ù	Ÿzª?{¸'!1ÅÌ?œ"øûÏ?˜U³3ö1?î¬W®+Á?u‰ÄåLË?iœ@4oë˜?[£d˜Ñ?£ ÁÛÜ1?Ž»»M5¢U?íWùã¯E?›%AÆw?‹o´5)Â?I+¸t?±Ò@²«A?›xKi€AAGN4FGL J1138.4+4857?ïÁG·¾a"@P†­-ËÀ:¬¸ô¨´À<¤k'QÕ@€šˆÕ@ÛçòÛ?Ào\¯-€¿¢3NSÙØ?áz‰hÉíõ?üâf´êØÑ¿ÙÚW¤×J¿ì`¯7¿Û¨üct¿ìåvã)Û¿ï÷³•Ä"?™A_(…AGNfsrq3FGL J1138.2+4905GB6 J1138+4858?ï­ó»•$?ŸÚƒž'˜?^mlo†J?`–r‰zŠ?€µc´»J"?Ÿ'mÏ+ñ?ï.Ž½êÔ?•ûM'ùÕ(?|ÿcÑJZÎ?…:º:ã|?'îOQ'€?—º sD?íí[9Prx?›R"Ã
RÆ?–¶fì¹ L?'G(ö}Ò?¥ÏôœZ?"tŒöÚÿ?ïx$~[òç?vÿ
I'.ì?…ÊQÃ?só‹Á×]Å?y˟¡S ß?_2S¯£?ï{Ò=œe?¤úøc'e?¿$	o?‡¯$º,]Â?~˜Ù÷"ê?…vh˜îïz?íâÎ|'æ?®TQ4}ð?–rÇç˜?˜7³N
Iç?©ˆ€%z?§Wï^ª×Æ?íâ鯼? $°•\é¨?š0샌Â?'xø	?°Œ­—ME?›z–wÔU?î:ÄKÝx?K©'Èæ?¢G¢'ž?šÐx¯½h?"rç`ôLô?€²7Œ"'ˆAGN4FGL J1139.0+4033¿ï""HC)@Qzµ^ñýßÀ:C¬­r"rÀ<4cʪ³@eMÌg@ŸžEÐÄ©?Átˆhî?µÚçÜr²?ñ¦+]{Ü@Á¿M2bÔ¿ëv_ß
¿ԕOó]ZN¿èƒ_›q
.¿ê"ö^ìtˆ¿ä˜íÂeÀ¤¿ðAGNbcuCRATES J113903+403303?ï÷ç"Ö`l?DA¦¤ßò›?*&bOÅ?õt0Kä'?IØhÖ¶,[?BNáºäö?ïÝÕÿâŠ
?n¯oÍúëŠ?A/éá(œ?J¯Ì¿ö'Q?mätŽ)>?j0Gú¢>?ï‹w£¶º"?'nw‹‹'ª?hm¢¥ï3?r¿Ö"«®ÿ?‡®i;°?~§zÆÛG??ïÚØ¡?Sœ.¯ÕÃ?P²Ç&ht1?7 ¨"Ú…?mš‡É2?Q7^Ó¦<?ïôêÁí?Ooe>'H?/®‰êFÔ©?%ŽÉ{ö?R6$þ´ÊÑ?L¦–qaè6?ï"DIþH<?‰Ë}±Œ?R*Çoñ¼?_¾?HÖ¡?ˆ©"'fHË?‡ê¤èÆí)?ï;®ïl4?‰Ɩ\5Q?uõ¾ß?{R‹
é?"X¬Úã½?"«ôÅL@o?ï€9ZáðB?uÆÓ÷æb?m7ü¹)!ü?\Iç…Å-?ˆ£ª	?rÚCn¼ÝAGN4FGL J1139.0+5530¿Éƒ²D¾Ôo@M_â?$ØýÀ;æéóN@ÖÀ=8C=lr@"ì¢$'–H?óÂ}qDç?Ög†aƒ}£?Î1·ÝýKÆ?öäí@	Û@gÿtißB?í!¼{¿ïÿð`OËð?ïú­EH­?™Ü8{$A¿•↦¿ÙsË©·AGNbllRX J1138.9+5530?ï!ÿTg?´¼m)M?Q#š¸h=?EýÖl¢,s?š­ÝR¾Ú??´€»P™Ò?C?ùª³w?`†3Æ	?hÒ#+.Ô?ˆ¹»?_%$?Œ¸sÒÊ7¨?ì\y°¢Œ?©{îDä?iñõx*Â?r
ëI‰è?¼L¢Òʵ?©Gè‡I}%?ï3ø:8àò?{®³Åz?GiŒC²°#?8"@P*êÈ?˜Å¬V'…o?{K‹wÔ`?în¦wE(?®a .Q?^ä;€[õ?V~
؝s?¨xS‡¡?®-"ÙX…Ú?îñ³Ï®\'?¥ª$H!6?hà<.o*6?y+dê[Å ?ž­~—!á?¤y·"¬ØZ?ë:ˆo®A?°6jèp?oÚ¡À'S?s±w_ž¨M?Ã~®sgÎ?°O:`/1õ?í±'úã±?›UÌíkR?SrÀ"rR?W/ºùRÌ2?²& "¥Àp?›A[ÏlaAGN4FGL J1140.5+1528?ì̱8òÕ@Qu'·þ	À:þX;*xzÀ<†[3,}7@"«Hî†?ûŽîDì™?Ç#KŸÐ-?¢8¾Àù
?Ú'Â	Ð8@Õ̉…û,¿èÉN][$ê¿ïm"Ãqx?æ»ss•#¿å·¤ëàŽ¿"Ïюþ`¿ÓÏ-"óoNAGNbll3FGL J1140.4+1529NVSS J114023+152808?ïׅãYV?¶8!ÅÒ¦Ž?CÊÐñÅc?6µ~"ž´n?¸»NÉ\?¶:K².[ ?6ü§—?š÷¸dôÂ?]Où¢£Åv?h>üìWˆ#?Šô3º?š iÝeL?ï1Ž(³d?ˆZÒé¯L-?^ rx,áY?L?¡õƒ?›7Ç:Êu?ˆ-Ú)B?îäÜIRÀ}?"ógè²áˆ?UÖÄnȧ?MŒø€ 
?¡…CìÖè?"¨ÙóÒ?îâü|<çg?›‰¿nÛÎõ?SÙ\j ›?EC|ôþ%?¡1mW¾¥9?›U¾½.c?îõ…v)°†?¦Gø]¼w)?eóOÏh`ü?tî/1¹?žç<'`"?¥_ËUtÜ?î#~Ô
?š‹€ž˜Sk?fx×ßb?fuÜiç"?¬h*¯ØªŽ?™ÂãûŒ?ì£/áÞƎ?¢"Å¡ï°P?f€U|;–U?eÌ,smc?º2~AúK`?¢r~þCÚAGN4FGL J1141.4+6805?êÂI¡3ÁÎ@GÚ.	þ†ƒÀ:NjY¹À<Ž-ë˕•@ ÏU¢Hê«?öd»®²?Ãß\œc"?Ðñdûµ@èDŒ÷ʧ?ûº¤¦½ïd?ïåôñ¯e¿ï²¢´ËNH?Ž±ß¿È¼]¾ÍÖ¿âT,Ý®œ`¿Ïo¬ö˜£%AGNbcu3FGL J1141.2+68051RXS J114118.3+680433?îÜ€ï"?£¯UŽ?ú?ˆ'[ÞyÒ½?‰\Þ­hç?˜;Áô—ò?ÊY™¾s?î@"Š¼?²ªdSç‰?—*yW-.$?¦¡kûÉý? bÊ
ڎ?¡þ°n¤ Ò?ìYõÒ"5?¦v"…´?ªÄ
'ß+Å?ž*
D·)?¯œ•²»Eê?®:'n?êóßP2ˆ?¢02¯¢?›G&K"(?ˆ¸m¾K4?ÀǝÿÀü? kxy,tz?íÕzLf#å?«~Ð ±?–#Õѯë?':äjhÎ?§–šR$…³?¥n^T僪?ë¢í*eY?Đl?± \\|Š?¾°Ž#ó?µÊŒ9`~-?²Ù:ÇMÈ:?ëæ­Úªl?©,zÑ:A?²Ž¬¹°?¢/(¨éäM?µZµŽYÙí?¡Jɬû®ß?åÜÆ1¨Y?µÊúP…×Ú?¥d1ÏM3#?Ÿú…£µª±?љíc½Œ
?µ•ÈнAGN4FGL J1141.5-1408¿ÙÀ«gˆ‹@F°Bž
A¢À:žë¥ÕçÿÀ<w»dg@ y‰®¿ñ?þãM­1üÒ?ÁBÎ[ÃO?¡p¡æð?á±ý2Æ&@
;"ÇOŠ¿ã7a–5¿ã,o_3l>¿Öf9ð¼–¿áòʍWkø¿Ûï½µ'®¿ß¤õî.FAGNbll3FGL J1141.6-1406NVSS J114141-140753?ïøR|&??~9N¨?'ogÞ)?Մ{;Ò|?JÜæÉõ?9ÑCÞØç?ïåÊù°?iÒÃÍBë?5e÷òT ?Cp¥G­?hC'>ׯë?eÞæ…P¦|?ïÇæMì?d[$ck›?LW{²Ô%?3¬Ôä±?xôgOµ—?c€s"·†Ž?ïÁ¬"ûf?WF|êå?A¡CO#P?#Q}™©š?|õ•Ç8?W+¦M¼^?ïñ'PÇe&?L7r•O¿?6¥0VÐ5?(¹·1µ"Å?W2Hm\C?H+õVšíØ?ï˜ÓžÖ¢í?…j*Cµi?N--÷¤îD?WkN	¡2?‡èEfKz?"R˜¯µú?ïž{Kƒiµ?sèÎs"ß?TÿÍæ?D€"oéY?…ÁK¹cô?s	×â°?ïH¿!œž?wÝY Ò?U\lÍ;½/?Bâ¸7S²?•'TúÚÜm?vØ<bÉUAGN4FGL J1142.0+1548?ëŠv´oçL@Q"¿aª?À9˜€£ÿN)À<7€@,?ú@rŲ|>•@zãËìÓ?®pC£²û?†oHQaÛ?׏ó"
3`@ÅZ»g?קּ'›O¿ß¡D¾uñõ¿å`½§?õ¿áVÄ!Ølé¿ãÌ€ˆ¦'¿äŠšXz"AGNbll3FGL J1142.0+1546MG1 J114208+1547?ï[œûþq?‰"Põ¬c"?e¦m»2†?WKåmïÒú?'ÒŠ•´v"?‡°ó­?*e`?ŠÒ	 ð9?f1^­ñ{"?t1Ž+î?†ˆÈÓC	?…Ôûè?î…íaº&¤?—"Mçpec?ƒB_&¨I®?'ÉDNX'?¢Ð'-éÔ?•kҍ¶In?îÚbõÌ(?€Ú&9îä?"p¸
u]?ySÉN'³?Bé.ŽP?nv®¿ô?îJO§]&¢?ãÁ¨Ñº?K	Í	Û?s_¥
â\ÿ?§q¤N|°m?›;GÌá¬?îÐç+ÑG¹? ÏX͉{¸?xmã&c=¨?'ö¼Tł=?ŸÇ¡Ãqa?›ýoÁ~Æø?í6ÕrÉÝ??¡ŽU;óU‹?Ž9£2÷-†?†QKç?²' .R? J°[¼?í}•.~?™?53¹L?«	5_'Ÿ›?"›æâ–?£^ñSÊ|?‡õÞ¨';ôAGN4FGL J1143.1+6122?²ÀÄkÂUV@Jð² yLÀ:dIÄo0:À<"Ö"Üs3@±Fúæ:²?û͓fy±?Á9r½aÊË?ÐD¾ÂH@=À@ÍOª@xKôL!?ïñ­!5Ú­¿Ø´EíJ¿Ö˜"úUò¿×®«¤‰Ø¿è'I†[Ï4¿êÆ|†c[ðAGNbll3FGL J1143.0+6123GB6 J1143+6122?ïË·›ãõ?tñØ´‡h?tQ6yôã?r†`!¦Å?WKîŽf&O?OƚF0´?ïÓ3ï¤EÎ?s²'xHŸÚ?O<lkj¯?WÉ)×2?r~zªy9u?oÞLªìë?íÎXW|`?¢´²Ø7—¤?¨ì>N'ªÚ?¡ܖ¯´'?"\xq˜Ù?Ž­™˜ÒPC?ï´øڔ-?^{çµæì0?e_b+½I×?I£ÞÑïĤ?zÓá¦êI?WžÄé´Ó?ï_Äê2í?ˆÂyŠ¤?†"vW+R?†/µˆ	9À?h)HÎýá?bfz¥9L?ïl)e÷M ?'°B)O—ˆ?c÷ŀFœ%?so³õðòn?÷µ%2¶Ù?–ªÕ?ÝÈ?ëßÔô0
?­¯þö?·Ñ?¸µÝÐöÀ ?©˜Ð™P—Ÿ? –õí¾¬?•Î‡¥	ì?ï>:*ü¶}?{˒>IOt?wèÁÞÓÓ±?cq¹¿ ‡©?'>Š Í!~?w§y•fçAGN4FGL J1144.9+1937¿ïÿÁ2Ýn@RAÓØZÀ:byz?a?À<Íùóv…@y¬'˜ï%?ÿÑ!%µ¿?º'ú E?~qB"ãÒ?Å6½+o"?û½'(z?ïL¾õsµ¿ã¥óD/Û¿ÒñO‡¿àÒýž%ðU¿ã›šu%¿ÏB7]xêAGNrdg3FGL J1145.1+19353C 264?îëEkïè?¢Ð¦YÈ'´?f»SÜØ©ì?dƒ®Ÿ´ì~?ŸÅ¬ÓûBÁ?¢KÿÙ?ï`¾Š6G?'ï§bòøâ?lX¼àJ ?p`¤$—?qЦëß?Bo	yÛ¡?íç,TÐD"?¡ŸÁÃ,°¥?x.YRU?€Iy­(_J?®‡o‹Ù0–?¡˜RRÐ`?î7Ðç8³Ñ?"Róɺ?'áÊ´?sç"»x/÷?£vfhî?€J•ñ¡?íëYØcƒÞ?°Fb§úaY?x&R'Õ¥m?y[ìLàR?®E˜%%Sw?®ÓҖ—3?î"b''k'?«êuýxµJ?yþ£ÕvÛO?†ÿBï't?¤z	Ü ?ªGÈÖ#?í[•å&'B?£Ÿ¯;Ä?y[yynÑ?{Œ-ÿço?³'ë"k?¢õqWl^´?ëNuž	¸?žÄ¤ïˆX?¥ì'¨ïÇ?Œ©4%Ö¼?º–d<â×?™G¡^œÞíAGN4FGL J1145.5-0340¿ïM{ì	©@K«#c²WÀ;¯ä	)tnÀ<ßæ Zé[@ ½'³K?ùÌ(bÙ?àèä?°8?à'õ|ï>è?ýƒîÑíž?ûîi_jÖ?ë.2x"P¿ïÿò(¦è7?ïÿVW$ª¿Ü^äq¯¿ãü°TDz¿ïÿÀäa>AGNbllRBS 1029?íhÏÖÜ4
?¶áùA»Z`?qÍՙ ¹?‡ã›òï‰?³§Ôj±ìÐ?¶µh"
)?î®9QïË?¥±Ÿ¹ˆ?‰ãä@†ØÍ?—E Ø"c?Fã§bH?œb°î,Ài?ë(ÁÝÿ>?±@wzœ¥?}ú#lӜ?€²OyŒ?Âm*й‹?±9":âª?ë<í¶s¼]? ¬WAh¸?TDƙ?…Çõ3ˆ˜?ÁÀ£¸p8?Ÿ¹!ö0/?ê…FÙá¼?ÃÂ)-©d?…ê×ÿ?"k—D¬
?Ä°ªÄ܊Ò?êÂ:;~ö?ì2®(þ?¼¯3,Že?¢x¼O
?®^$ðõ?µâ\2S	?´˜KÒ?éœò'?·ô±!³?'¤ÿŒfM
?"–å—ñd6?Ês<<
6)?·ù+œÞ??æ9•¡	?´QIÒ×µ?0'mÝ?Žla™©˜?ғE %Ø_?´}ŸQ¦AGN4FGL J1145.5+4423?á_÷·\"@@QèÑQ­À;z8«B9À<ª"á{°{@ÇRÏ۟ù@oÅÀi<?» ¤iT'¿À*Ðù'7}@äpùg@.°',ä?ïŠ[…~¿ærùпãÓõ €"Ž¿ç
:'£¿âŽ7€ŸÍ¿ðAGNfsrq3FGL J1145.8+4425B3 1143+446A?ïÞ²Ž™FŸ?z÷ ·ýQ?Oã.SŒ÷¾?Kö–Ï^… ?iT¦º´?y‹@îæ0?ï£á³±W?Æ«~&)=?`bJBYnï?oÍkã
å÷?'ï}ý$?‡™ßh"³?ïB‰™¯?"´¹to,w?nhñ¨Î[?n3õ±£7?"ᾜ>É?'ï71¤Ð ?ïv©Ä×Wb?s%õÅÚä>?w;ˆS5†?d†ÝîŸè¹?†·Ê"(êš?mäýœ(º;?+"¦É6?u‡­[{=?d)¡)Qþ;?[HÖäŠ{?w¥dýÕ^9?s'úÏ Z…?îû›qµúÎ? c-+DAò?t[L¾ï?ˆ¹p'c?›u¾¡z‰j?šajryŸ?îNaM‰
?"ÜŸ¾üÉw?ˆë¿«Ê?†ȓÙÆm?¤ÞûDü«¯?w"fê`?íþÂ'þg?"ç²å!?•Ä&K?‰Tl3œôõ?¥Lü8vú?Œù_
<å AGN4FGL J1145.6+5552¿ëÛPPØé@Msb¯È°À;¼±AV¥À=	l«$™@çX"Öĝ@=m;l½˜?Ìþ0­ï?Kèü}ÉjQ?}âkÅuëj@70Ûê÷Û?ïˆ?Õ%¿ß"ä"'ï[¿Ø|Õ¾Ž¿çÀùYó']¿ÊòëÅ`qÛ¿ïÿÿ&¦³AGNbcu87GB 114248.3+560915?ï˜`2‰ƒç?Š¾ì0â˜]?`<ˆ²Æ°6?kl[¯3£?…ØÑ$æ¸]?…0é˜9¼?ï ~ß^B?ÏÂÍ#ó?W¢š±åö?]ëè}K¿û?"ëôÙ{ôÓ?C½Ê V?îÑ"}¿"¡?'ÃÚt?}¹«¢ýÐ?'<œ›[*"?žmE^Ì®?mÛ<Ꭴ?ïÑI.zÅL?Y^1/k15?HŒJ6*‡ú?6}Ü
'U¢?tIߚùKÌ?XѤ‹§?ïA.菏Ä?'FO?iÔdDôù?g?qÝ£kÎ?"Ÿ–b÷SÜ?÷ŽFž,Î?ïÂlõy? î2â¦4?`ΦÞ4?h"½3í
b?š&˜¥eÆ'?ŸqrÒÿ?íÀ˜ÓîKš?˜—¸¼÷!?†&é"ÛŸã?…Ë6­bº?®l¸`ÀEf?–@ðE¥?ï\B±*"ä?|¸ìèÅ'?ac±¢DN?Vw;2t‰!?'K3®Mó¸?{íÈØý-AGN4FGL J1145.7+0453?â"'¿}2@Og+©ÑöÀ:ìH£ÝÀ:À<t·×rB=@øW8ò@"{?;2?É\–#û¿³waì?çšr­™@ҘÛпÜބÛš¿é <€¹Îÿä†(¾e*ý¿íѾ¾í9?€ùu2˜?¿ïåﳁ¢,AGNfsrqPKS 1142+052?ï¬ÌXLŒ?¥1¡yíÛ?bP
QæM?}òp"|Bó?€8çf!æ8?¢pÞw_¬?ïÍb¤Ãvë?|ý[0j?Q9¶Ñ?e!"ªk£?uŸÂC?uíl^0åŒ?îá±s*.?"£k£"Î?lE±ü™—?w<TX¯?  ¬5–?"KEëÊþf?ïõ…÷Xð?B>½<_%?$q>½‹šÑ?}Õ%&œl?SJÌ_E1!?@¤ùîƒfp?ïÂkJ"f4?'µ0µB­?`(Ô+2Ê?c<xÅNTR?vµð­Ë¬q?€ÍRþZ†…?ïä\">?•»žnni?Zï0|°ï?tâT>r??Œ©ÐçO	?"iŽÎŠH5?î58Ã.Ø?—gºåžÉ½?už)sÞHq?y"Á~ë™?©ø®›?–E'¨¶!x?ï×jÆX¦?g1Šáj?E v­?G8…ƒë8?qÑf¥Ö‡Ä?d—	ã€ÝÔAGN4FGL J1145.7-6949¿ÙW ÈJ~À»?l&šÀ9èn"2QŒÀ;Ä]¨QÃA@c6æÆóð@S'ˆ?ŪD'?Ìûúâ´À'@é¨ÛUüŒ@\\¥t?î¶ãâ.V¿çÜ¢˜E܃¿è›¬>ÿ=¿î$Ä:Wã¿Û7ã¼R,¿ïñâ0`†AGNfsrqPKS 1143-696?ï͖êÎћ?rëÛ¾&Ë­?GT3ô"K	?K‹Ê?©	?vJ%©?q~;ÇÜ?êêËþŠy?¾<"Ñzÿ?z'ë|õg?'åŠ®?Ã!y¹ï?¼¿t¹T8Ö?íÒL8 ?—¨¦ÑX¿?ƒ¥¨"µäf?}g@rã)·?­ñ͆Òà?•ËI"ônQ?î©a‡«?}zÕ©Ø:›?u	Ü^•®?]¿<¸br"?¢ÈÍûÖ7 ?{¤ù‰lD?ïmZ¼¢?sú£?RTˆsN¨?MªŸ3ä
?'4¨¥¼lÌ?5vô)è?åžjNÛãÊ?ÉFh'}ü¹?ÎÅí¬ä?—[̈́xb?ÓÊtìË?ȜŠ˜RzT?ë² £…øõ?¤^Ù/TÙ?"ù璉Ê?Pçо†Ô?½0³çxŸ¤?¢Kw
™#7?ë)3l,è°? $m85Ó?"}àØ&Úü?'CÝGìÅ:?Àëv4~{ ?žzkAq®QAGN4FGL J1146.4-3327?ˊ@~RôÍ@;zãâ"À:æÄ©Ü¡À<€ëaŠR@26ï©@íàBËV«?Ïڿԗ?ÒmõJ‰;@;ç+y+?õÑÊWÒyà?ïõ/¢/k?´€îýÏ#>¿åÞ¾Ò8F˜¿äè)UJµ¿ïñp»Sþ…¿ïÿÿ)@k*AGNbcuPKS 1143-331?íZá#,;.?¬ƒØù<'µ?‡vk‰i_e?ƒUâV?²:)t' )?ªÐy´|?é–_°G?½t4ù9šß?ÀšÈƒ<
?¸ÞYbØùg?²n'ÔD
?¤ŽI8Á7?ì"Hch?¡Ëë´ñD?£/‹.­ù‰?"E\¨ÿ?±Ï°%#z?œÇ'…'‰?æ'þÎbï?¢(p‡]Ÿ?ÇÖIrú? «Å^L<?¼;w'öóp?"nQRA?êß؍uI?µºU'¼©?˜;Aß_å?">"E<Y©?Áy5¢â»?´»ì·-;=?âŽÒ:lYè?ÊWyþ7—¶?ÒÆÇÇvÄ?É@SRôÕ?Á)†¿ªÙ?³A³váõ?êm1±¨Ùþ?¨øèÎNñÄ?­Ð˜T&‹?%wìrDñ?½®&j35É?¢âLeEø?Þ\UŒa?«¬l"¨É?ÓSeМï?¯|á÷4Ë?Ì¡¬‹lbÝ?¤ê®r	UìAGN4FGL J1146.6-2902¿íÄiÀ@?¹Áç–|¯À:ãòènÀ<Œ°"‡áá@_ʇù@<'Éä»?̟á²7Q?ь!f,/@부#§@†)ç0'?ä1£{š«?îúÁ'›ü¿ålÉVö†Ú¿è´Zåÿ¤¿á˜'Bdÿ¿ïûM³çùyAGNfsrqPKS 1143-287?ïcém†/?'¼[®Ï¦?pGís_?fA_q+É?Žâ¨¬v?ó^(v¹?ï3|hJ0?"`°7ùh"?€b#Ý;?'µ.ñë_?'_a·c?‰Íá"Xë5?îÌBZºØü?R÷Ù.Û?‡/ÏU²î?{"•¹ã?šßÌø¤h–?…˜8¼?î6'•»µñ?"Œcù–.?˜›9ҕ«Ò?}Yì³v? I9½€?yý¼->8â?îi†¢­$Í?™?uWëq?‡0»£s{ç?€f6»áì'?£›fî¢4?•Ä—º•ii?íþ(\óÿt?©nÙB?"°iS{‰+?œ«‹jŸ®?¦EEŠqà!?Ÿ.Lòá"K?íŠfæ
'Ý? aø3?›)ÜïÅû@?"5Šß6Ä?©Ä£*äpˆ?'åÞ|Þ´?ëOÙfÎ8?¡zñ,»ej?®‡Ùe§ó¦?›²P}N'é?¶=K	­q?"'*‹Š[AGN4FGL J1146.9+3958¿'ß«ÎYÒ @QÝ÷'j@À7À¼O§@À;ŸÝkí@ådÉ-[@"ÚZT	m?"Mé=Ï?±/à~–š@ɝæ?@ZĨ»ö¿³ÊÅáv'$¿âáT¾É(þ¿æHmWoÈ¿å'pjÌ&µ¿ç½jΪó¿éÌò!+ûAGNfsrq3FGL J1146.8+3958S4 1144+40?ïâæqâ=?b½p•<³R?Bûº˜d2??Pz'?hy€r̾D?`'(œ*gc?磻Q®sp?"]X»ñD?Zñ}Eüêœ?j™[S?ƒ8»älX?¨ZY?Då?ﹶ Š©?€ŠqV±ÿ?](²	L?n|DîÍJÈ?{ÚÑËKܺ?}
¯gºŽ?ïø)¶¡?6U}e³?7 ƒDKì?&r«E[—þ?CÈâÙLsC?/Ϲ½õ?ïÒ³ç"¹h?ru®CNþ?9ì@E?2K];ªÌp?um©àfm?qÒœՈ½?ï,ᓔƒ?žz}œ#fÖ?gË3Tt+5?t÷Ékì}?—jg#'è?œ»ó5Â.¹?´¥'†?†ÿÃ81F_?cLÜT™?põKŝýÛ?†Š¿›'ÁY?ƒøg!MµÇ?ïë‹&9O­?Tfuė
?MÊo[†`Ù?B‡1…»u|?Z{k?NÐo'KAGN4FGL J1147.0-3812?ïA®fkÊ@6ô	å\ËÀ8v`' ×À;±d¾ÆyÌ@là{U`Û@G
=p£×? Î»do–;?«ð~ã"õ@.®@ð‹@½áÓo(W¿Å*F$§5¿àÙ§'æø¿ä‰¤úì/¿àõo]°à2¿è¬übf§¿àÍ7¡AGNbll3FGL J1147.0-3811PKS 1144-379?ïôAšîÈ?MÄ{®ú—$?+ôMra4æ?"þjn}Ë?S`ó"µ>?Ks=ujC?ïÂçþ+•?y¢¸4&ˆ?SÙ2°eÆ?Y‹¬5C~é?yý¿v^"S?w	8‡^Å:?輻õÇ??v‹k9O?^wðN¹?dÅ0î)Ô¾?'+ùҌÓ?|tƒJûf?ïÖ*¤ÌÜ?TSÜèÊ?U¨Ê¥k?:IbQAïQ?oöüHa?Q:ÝRBx?ïì6OÜ?_Ÿ³drý˜?1%y…J!?."ÜS?aùðL?]i.© ÷¬?ïP© f¬?˜ÏŽÓTìº?j³°(ù´¼?{,<4ñ´?'§ôËû]Ý?•ã×_á)?ïC(vkÂ?'vi'"^5?j›uÿJ?s/Æm(u?"G'yAÐ?býÏnÕ°?ï¨øsø(?m£í(¹'?g—otŒVÖ?TSwë+Ú?€eùØ>]?húÀ	ù³ AGN4FGL J1147.2-2627¿íØ2"œ@A\1YÀ:
'@ßÄ À<T·«c@2—"@÷$œ—zÛ?¼]v}µ¸^?»´jÀ¾ ¸?ù]RV)Ž@ìéõýr²¿à'#€Õ¦¿ã{V'Ô?¿èÆB¤À>I¿å'EØQeM¿ëۙN?F¿ïíœtÜAGNbcuPMN J1147-2625?쬋GW"¡?Җ9­ ·›?˜,À9'R?²\˜ÿû)U?´žÓë$&?ÌÏœ-ƒØ?ïÞ Ꮦ?p2.à'?AÄÞÇæ?M"¶"9€?lîòyÍ&?jáý»Ž€?ï½ÚÈœ?p~‰!Ä!`?Yœ{2:¹´?VHÇ:*å?z«ÕÖÀ§_?n|þLYqw?ïãÒRÑ;Ð?GŒEåƂ^?M[@¸7?/ñn,O¬Å?dÖÝ äw?D¹ŽžÂ7?íp`ºÙÚ?Ê¥å5?'-313=j?©Áx<Ê:?¯ãZÅØä?Ä7¦T½òi?wIÚ?…%ƒÞ?S³ä›
ï?bOA•y^ô?"åeœ}SÝ?'‡q\p?ïŒD´ê?|MJÉÅ`é?cO–Z½ÃG?`·RßÅQ?ˆíP¬¿?y«ÔšL£?ï­Âב³?kJˋBG?f'^G¤%"?R%~|£7Õ?}Õe¤€|?eøøZ®•AGN4FGL J1147.4-6758¿·þu$§üŸÀhaýKÚÀ:I:MÙ§§À;Ë
ù½Ç@_‹p¶÷M@§ø-ýi?Ì@x@-˜?ٿώH,¿@žÈ~‰rÛ@uœ9\¿Ùçwþ"E¿ãRôÏJU¿åD(Müã¿ê­x:¤A¿ïþûž‰s¿ãlqãr*ÀAGNfsrqPKS 1145-676?á
§Uf[K?ÀùfWf³?ŏ¬KßÒ?´'	͉5H?Ó"Û/CÃ?¾TD5Qé?Ýʃ•åô«?úÆo»y¾?³YÎ0,Ì?ª›{¯|D?Ýr¥öÃ?Â^Lž`  ?âfDMóäû?³m¬â?ÂPi`'?¥ÅêA""{?Ò%O/h"~?°¨WBI5/?â#DiL°ï?¤¹‰yëó;?ÁzÜ¡ù[î?˜ÿì;?ÒüÜið+?¤×C
{?в'½çµ9?½ž¦Z'?Çx¬ŠÉ-l?¸¿{¡#5@?áÈÀþYÚ?Âæähû?ÈÜ
}ñ¦?ÀÀ="­n?Àω9=þ?½
á™Qd?å•p'?śó'ÌÅ
?ÕGu&•Ž?²Û6CŸA?ÌHS¼ü±?±³Š2RË?ܲf¯Œu?µM]ŠWƒá?͑8A?£à•ÿÉÓ?Ï~]çDzâ?¯âvû[–Ú?à¼#¸ƒ?±çœ&©ÇMIXED4FGL J1147.8-0724?ï'L£œ§Á@JßeUÅÀ9yæ'æÀ<TTëêŸ@d"ZD[@¯¸õs~?±òù²3†?Åä=;IØ@Ø\$ħ@~¹*³?ïÚua«ì'¿Ùº·Á¢Í¿çêßÂrÖ·¿ç_XŠÛµ¿æ…Lp¿ïõæÁÀ7AGNfsrq3FGL J1147.8-0725PKS 1145-071?ïíR›Ù9î?R•ûoñA?N?ԙ¸i?D57®³ûq?V;D;{¦ž?IyEdÊ/?ïÕºj'CÄ?s;$xð(µ?Jå/R,?Zý!ɔa3?qàNLëN?pJ!À#Ûú?ïo{&֝J?…Å'ØZKZ?yµ®3¸?{ëØ$Gž¬?‡F_ Q"??~Y20á¦?ïÛ*r'ºJ?Q,úÕ3Ѧ?Yþ{çq.½?@œƒ'$¶B?gÖO'Ì/?Iâž\UM0?ïá5\ƒ8¯?'I96,äÇ?W £½¯õ?bÑ^Àt`º?búQž7øè?{ñý~›K?eæ?‰)ËÀE?ZlL8x§?hÙ!¶µf…?‹Tq'­?†Ï—D-?îógáe¶?"2¯¥c?‰n.è½ò~?Š[=GÇ…?"Ûì`¢u?ŠS10˜‡?7‰·­?pb§nò¼?s>`"ÛÍ?_Üö[«"<?€~ÜÒ?hôR€¶áAGN4FGL J1148.5+2629¿Á0øùÙþÂ@RýàŠï²«À:–°ä+ŽÀ<oÅµW@£I.G;(@§±9ÉOj?ɞ¥2?¼HÛæñN?îõù`½°@¹î£·*¿ÛBž54À¿æ;T»,¿ëSà4éí¿èvk—'ÏR¿ïÿ³©æ÷¿ïÿè+ÍäAGNfsrqTXS 1145+268?ïöÞ«hñS?Bö*ov]?CQò³J?;um¦d ¡?A4EI8º?3ôÎ?ïØÜW¯>q?s}¥KÄC¥?H	rœ6?[ωÉύ¹?pŽÒ÷ÏQ?m^Ùªti?ï¬ælIîû?r"ÇàšX2?_F†<·õ?as`ì^ú?€Ý")r.?páî"?ïãØæû;?LU!ˆŸ&?Vٖ‡]]?<×	M Ãñ?`ºM}¾"?D(0 ˆN?ïòëÜî"?R7J؋è?PŒ«›7?Lý–¦š'ú?F²ù¦
­J?B\Š¤Ø§\?ï€/ß&ý¬?$rø†i/?`I‹"T1?mâ?Mda$?‹á¥zb­?ˆÄÇí*j?ï[2à@á¶?'S×V2Mš?k%pÅl?k½L*÷ú?'7_Aø֓?€ãú¸XÒ?ï¨-™ýRã?o~¬ø(í ?q› dûáo?`ªÐ^?zM'™šý9?f¹À•ÜAGN4FGL J1148.6+1841?ؕRÓó˜Ð@RQ'U°5½À:œ2ƒ
À<'HÌ!¬"@ÚÏE"@7›x¦?Äuƒ9ÛÃá?§e"ÏãÙ?ãO؅g³n@Æð)s@ê?ìô´!Û¿ê&$V÷]š¿ãÃQùÇכ¿×$:ýöe¿é Ÿ>À¿ï÷,ÊxAGNbllTXS 1146+189?ïÍÅ£7Ó?h÷·§Éœ?Që‰wù»â?Dþn °š?t¢Kù	?fÝ»)²¼?ïÖöæjœp?sywTÉ=?C¨lâ¡M?O<,š×v
?rŠö_`—?q%µÎ°á
?ïŸVÔÅa?xZ—" J ?\èçÚ?gW½¦F)Ë?"-ýµc?u+R@å±?ﺊ½³ª<?\0|ž°á?f¿ÐÕ?Gðicr?w¯ÁL.¸j?WK—|Œ¯-?ïQ©?‹h>¸	ŒÀ?kÑaF÷?aïc oi?'x'8M%,?‰ƒs'sàw?ïˆ!F̘?‹ÿ"#Z;ú?TÖ­üöæ?`Ž4¹Ä?‹\؋+sŸ?Š/E¬¡M?ï;(ëº+h?†Öjõ>ó?fô¸Oòn?k1rìl1z?•¼K}à^-?…*vcˆ£?ï<f(^Þ?wÔí.vs?~ê2êµ)f?f­zxkx?¸°%Æ9ë?s'¬%ÚAGN4FGL J1149.0+5924?ډY?·P@Kû`¿]xÀ:¼¬'\fÀ<—ˆü"cõ@S*¡iFÁ?ýØPXÝç§?ÑC¢A2û*?ÍwV	L?ö<py@œúåcǿᲈˆ˜À¿éu0™$ÿ"¿Ô£"ŸXö¿à—¢H"Ä¿ã…WWÕ©ë¿ðAGNrdgNGC 3894?ïÎ@ú¾o?m¥çý `?Tì«Kµ?E>
?z?sÚº›NÔê?kE>'HÝ?ï îê{UÙ?'N4ר<?XÓ¶ ¼ü´?^ÂÏóÿf?"©Î™KX(?'>Zcå?ï^!XÒ?}'9F@ØÃ?kéU¶/Q?eA/c£?¾ªWÿ[Å?z–¬ªòu?îÿ¾Bµ "?u¨´ã¢?yd²ñR<â?Z1@ë?™¯
î;I'?s+»j…Í?ïƒ*È3=£?•ûÆ·dý?c!ýšæÆ×?W5'Wôdí?Šl΃‡é¬?•àq
l Ñ?îñ%ð](X?–­±€J{?o
¨#?rpÎb»Äa?ùìîêÔ¬?"½m¼Ï‡E?î¬"-"ü?$"Ðã¨?y,¼i,àM?sUÏ¿ï7g?¢Eœò]Ž?Ž­ªé:P?í}ÒIŸ—q?'/t…å'þ?†¬ÑÌê=œ?stØ<•#=?±;Ó{‹¾D?ÿÊçI™µAGN4FGL J1149.1+2819¿ïµûx(R@S
†½ôµÀ;5º>TÏeÀ<¹šTbX@îÎxžwO?ú:73rô?ە̅0b?ЮrĘ Ë?ã ýy¼…@œVUi?첁Çë¼|¿í–ðÝMM'¿Ü¶¡gP¿Òòœ"%¿ä°Ëæ¿ïýYÝl[AGNbcu3FGL J1149.1+28157C 1146+2841?ï¸4qC0¤?|â›È'?NCmÑT•(?CBD"/b+?€¬à°á?{¹âÿ÷?ïͨ*'6	?xQÙl½up?Du‰Õß?O¢pÕMÔ?vª* "?vý+²÷r?îý9˜–Ô?'€¬GMÚ?k¿¸ü±"?s0<ê÷?œàÕË׌ø?)G.å1?K7·?iy|7oî$?UI‰éÿ´À??¨€zU÷?Œ3ëғº?höÓܝ"?ïDÐ\#ll?"d2¥0àú?[IV¾GÉ?Tk0pMT?•±_áª?"¾§œÆݐ?ï@Y_ÓáO? ª¿ºHC?X'ÈE"ÑÁ?f½éêpÊä?–k·‡`ôò?Ÿg:¯zí·?íáÆK\?žÈöæš_?roI¤È?vV*̌×?¯ öbÐã;?ž²6ÀÓ½?îØ>Èxæ?†WÙR8©a?Z"Ø1Nël?QÚ¼iÊ>h?¡ªåOÞ6B?†%՛‹2åAGN4FGL J1149.2+6246¿í'"÷©¢Ú@Juü–þµÀ;C`dÄ¥·À<➽ÅÈÍ@î]ìn@åRº·÷S?Ä(2y$?¿¬'Ó|"P/?啬¿ç<?üUŽ¿öЁ¿âVà±09¿á?-!¡:x¿áOÝO³¿ããY '¬m¿áVó+Ü'¿ïÿÿ)@k*AGNbllNVSS J114926+624333?ï×¢Ú¹?hû|óþb?SLÉïO?D}"9³˜?n¶ÁœéÂh?fÕÁ@':‡?(Œ!?"r.p«¹­?b0¢ê0:?d<éª{?‡ìé,;ãª?£²D³Õ¯?ï:k;ûj?ƒ¾Dj.o?t_){çfˆ?sq"Ú D?"šÕt_O%?Æ?óÀ–†?ï'rE9<"?j§3|Í?t	fÇdw?]ˆtíh}?…^»V•©n?g9L °?ïª>nª?zãhóDö?fG´›dâ8?^$–w¥!é?¼î¸xå—?wI"?î·sl¼ÊT? ¹'oI?u{»ˆdçƒ?€>È#c'?¡ÙQ¾¯?Ù?œÉYáÙàm?î+Òõ8"?'&¦Çz^ˆ?Bž¼•[j?{ŽéӝëF?¢Ü›$rËÛ?ŽêL<m?î[»6;?5?Q?0ïŠ?½Úi¾?{‰?y¨•?¢€Y¤B?‰6U&£øAGN4FGL J1149.4+2441?ì	Êó?
˜@R÷l7`¿]À:îY_æÌÀ<
ª}íl@ ÉêWÍ|?ýz¬(©l?ÎՑ—l™?Äk«õ'½?ùƒX´Ï?ú^/5L¾¿ê{`"¾ŽF¿èç6žË2¿àÖ|x÷c¿Ø]]¾¢¸¿äå}ºŠ¿Ò^(_ÀñAGNbll3FGL J1149.5+2443RX J1149.5+2439?ï2VêG†ý?·'¬^o?S†xÌ?e»¥kŠ–µ?˜|»:É'?¶âK—Hª•?îö·1Ta?¡ý*bª?€ÎÛHÿ5õ?‰öñ{'Nu?˜Á¯9jå?™ŽY"|ñ"?ï7‰tÿ?‰¼,µxnè?d›O˞Q?`¤W½ý?–{gq¬ª=?ˆ¯*Ðc/O?ìÌaA…Ó¶?"(+(ˆñg?–€%3©\?~Ï+Ì·~1?³üì¦5÷?'øñu+?îéúÐɺ&?«ñuOl¸?`ÅÏ1?X>ƒ±@xm? T¿/Æ»?ªäBJ­lB?ìô}Æ)o?½ß{¦¥y?–ϺW?£*yÖN¹s?²¨JSšk?ºWCUP{?î}Ix*D]?•eµ#~Xw?pðòžQ?i`Ñê¬{Z?¦
J%ÊL?"PÁ•_mç?ç]׊|+†?¬Jñ#šï?¨?vìr9?˜Ì›'wy?Ìxá·¯H?«é——b'AGN4FGL J1149.5-4029?Ê7=ïN×Ô@4Þf˜»MIÀ:(3û°À<;šß÷.@-' %ú»@lŠÅÁ@?¼†êªÙ2?ÀbHIšÓ«@ÑÄ2ÊW¨@
®"ѶkŒ?í€ÿ90£6¿ÅG³Gë|¿åÓ áŒwr¿ç'
~ß0¿â9ã¡$¨V¿ïÿþó…õAGNbcuPMN J1149-4029?ïéô "?U:ƒ¡šû?@tC¦ž³?4wáK.c?bÒÑAÓ>i?Rá=ºèì?ïÏõ}½gv?tzl®:W?R+G%¹?[8ö'€7?svIÌ¿n?oçƒéKa?ï®"qçEk?t'«ìàš?^ã(‡ø?[È:ñŠr½?€šþy
L5?o¸Ã4+ƒw?ïr$SW§?c›ë¼z¼Ù?tþÇÈÑ?R5ï™$ñ?ˆ÷ßÕP—?`Ði–Dñ?ïҕÁÄ¢?eQ" Ó½?T$½nŸ?LšÖ3ä»O?q­ž†*ãl?a¹$õ½çÄ?ïu">C\¡?Œ¾ÔɒÓ?j%Vبp?uHÓ¤ÉuÅ?Œ.';©?‡i°ä2å?ïk}»)À?"è•
TÌ?k·»³ÁÙ??i‰­'"ÓÁ?Ž2±0£±¬?{v·îI™Y?îj;BÔÄq?'Øç è?â䇴f?q×cDñA?¡ã'ÐÁgÙ?}éßNþïuAGN4FGL J1150.4+2418?ÔnXdèYh@Rþ€sWæqÀ8Ý^žšÀ;ÿ…ÄÐ	@
;ƒcÍ/@Š82vtÑ?¤ð?éØ?­‹ÊNe!@Ñ™Sù|@
H¿ "_ž?éT¯àÄ¿à
RÎÙí¿äF¼x{¿áº(»
,ª¿æ¤Ùžlg1¿ì~õ†÷AGNbll3FGL J1150.3+2417OM 280?ïç1¢a‡?mÉ܊%"?:Mb´­'µ??ý.)zl?e"±Ison?jXçp›?ï>ô¤?šÈ#*@_?ybOÄ!!J??ÚEjÊ?'É›˜a5?ÖióRŒY?覆8{?€ÒìW}:?\̱½àr\?hàèT<>?ß{ïó??~yä¼es
?î¸M
Â>?'˜]DÙÃ?™YÛ:9<?}`†sÏ?9ÉØ,¦?mH[Òy`?ïÁeÑs®+?vÀ³í`s¼?L"þIÖÇW?J«(¤Ï—?{¼w~‹?tž‰Ø?îع¦:£?¯Ã¢…mÁ?î²CÂI'? ¦Ýí	û?¦Ç×?xƒ?¥Ú尜¶?ïpé1åÞÊ?ˆEoy{?fgÎnV*Ÿ?ni¿5YY?Ž+¿ëJ¸Ì?…
‹ñ¦¦?ìÇö—T" ?Ù¹P`n?°Í½;	?™sÄ·™M³?¢|ûÿgò?…šÙÊ1!AGN4FGL J1150.6+4154¿Û'££@Q«øʁ˜òÀ8²¶d«{CÀ;š‹'!­@"³<Î?ùæ)_tڝ?¨î´Âٝ¯?º?©ƒ	@ãá!îgQ@§‰§´¿Â¢£C â¿ÓvÍ;Ý{Ç¿Ö+P%\Zõ¿ÔjzýÍÙ¿Ü-þ`BµÝ¿ä&œˆŒAGNbll3FGL J1150.5+4155RBS 1040?ïލ˜É(í?€8ïº'x©?Q7uTnUï?O$83­?hÖ¬±»¯²?€ËÒ¾ã²?ï´½°`k·?€ž¢¸ì6?YÀ-
ÞÙ?eù™BŽÓ?Y7ÎÖ@Ú?}ª¶r¦dP?ï¤Tìt¥?…eðRkO?l°,É-Ñ5?}Lî™pí?}s_Q€ò?SÂ=à\ã?îւ•h~ç?'LÛ«?qÞ>¢Ç§‰?U <è¿ú³? \Ø6?'†¼#/¦?ïÍ3Úˆà?pèF®mIJ?R?"‡\'æ?JcM²?tÖ1°hFr?mÈjÛG¼;?ï#ù]¾:ý?œ呥ës?pMz_?|5' ¹n?—yÎ{9ñ?™å{£<?ï‹C""?‹¼Û'Vl-?pRò'ƒ*?~–xڂ?…¾N?…nûß™ù?íw˜ÚŽ?›O­@ѓ?€"ì?ß=?l8և¤?²2¡ºeÇ#?›)cZ@´AGN4FGL J1150.6-4823¿ì¦•åsÑx@*…ê̒jÀ:,Ù=—ÀÀ<Uäßq@ZT4_®@ÕM¾Ñb?ėܕ—¬Z?铙¥X½@V́Mrz@uOVTux?ïýý'¶œ¿ÅŽ"½"u˜¿è6u¨"ÉY¿ïÿ°NçÄ ¿Öÿïcû}?ïôlj£'AGNbcu3FGL J1150.7-4816PKS 1149-480?Ì46"\¬º?Æ6ŽP1¾?ærkÆëj?ʳ …_ë?´:3d=?¶ûF=3Õ?ØüˆkØ?ÓnÙï ?Þj¬"¢º?ÒÊThsB(?Ã"®ËÚß_?Àá~•Ò?Úü©ÙÙ?´LM'-€?Øs¡qn*?³¿…Åßð+?É ®ãÐú?­çÕAŽ'?àÚØyåZs?»kR¹u¾?Õ×þԱȏ?¼úD?Àä o?¤• ¡.e?Ê.³ ð"Â?Ãó¸ÇÆ?æSòܚº?ÊH8?®ãû?¹
Q(ƒÛ+?·ïC[ì²=?Ç_h	B³?ЬÔNÌ@á?äÎ[CXÖl?Ó$'÷ý¹:?Åg*ëÚ?Ä?´£Ğ?×Ы2bº?¶Æ2«ƒ9?Úyq!­?¹—ª#(á?ËkÇVô¶ÿ?°ì¶L,Ô?Â[N+l?²ô?ã3B?ä9Ôk7í"?Æ.TTÂ?̽`%ã"?½ÉÝޘ¸MIXED4FGL J1151.3+0957¿ïcÔ/[|@Pï‡~äâmÀ9î{Üð0À<^RèÛ M@Xx]Öu@9^á6ç?³ê©ó¿ÇuçY?Ùæg¨…ŧ?ûáHÒ©¿å")uš¿â¢âƒw¿ç9iãÉh"¿ß?üoQÇs¿éa[?êx¿âðŸdß©AGNbcu3FGL J1151.5+0957NVSS J115117+095826?ïp0 m ?ƒ@îÄ+±?mªl3'?`§üvç¼?Œ‰QÖj
?¯TQ?ï<š ìÎd?›um\¨6:?xŠi
ªI?ƒŸÔd"kÉ?'J!›¸-?–z°»Ã;ß?š
­®?"Æ,¶?‰úP°Êø1?ˆ¹ÛI
Œ«?ž+ägüœ&?È]VSf?îÑsÒ­ú?€é™
U?"^v1Zû?y#¹‰ã??'s).Eº?qˆñÊ=ìl?í›+Š¤´?¥É†Ý"sû?‹‹BâÕW?{¢+P¯?¯ˆ%2Q|n?¤@íʸ?î	h½¿Ð?®L«½#/²?ˆ4BdÄô¾?'Mtw6?©ahØ_×?«Kñ^Qh?íVÆ®®1_? ‡ËìÌZ?˜ˆhµDG?''X"•}?®RÐàÂGð?™^ujá~?ì¯A$ý)P? MÁ‰?­™ÌE˜?™
¢gääÈ?§r!§öm?Žýê "hAGN4FGL J1151.5-1347?Õ;bFœª@GIÿ¼ä!À:+oðSÀ<L•¿ðEx@Fs´N?þ¿4"…ƒb?·ŒÍ|²?°s¿jc¡?ø õäKj@´~wTJZ¿åVÛó[¿Ÿ'gB¦»
¿á×&ø'Mu¿Û{–yS¨õ¿Üë±~è"R¿àþp·'©AGNbll3FGL J1151.4-1346PMN J1151-1347?ï༻j?V,w>'BP?D¹Œ¾hÕ²?1اFOèâ?j‡ÓRà¾?TJ¨W ?ïÙn(í	?q<tÞÏݼ?G/ðk°¿?PÌG8.:?pc–÷¾?l<C¾4?ï´!dv­?e('¶w©
?W‰°YÔ?Tá7I¦?€5¹"ÍX?`im`7n?ï"»¨•¾?a]aŒçIp?i
ߏ·ä?Eû‹´¿M?ˆ¹™$è|?]óqßèɳ?ï;ô¿Q†?e*‹e?Q¥ƒg ?A¹•%Ïg;?t·$¶Ø?b·fˆÉy?ïtÉ+¾°æ?Œ]Ïô*§?\M•z÷%:?c©ßù)–	?D^51¾?‰ÜGש~?ï{ä
';h?xVéýÿZ?`ò'ÿ€?N»~1èg(?€°*þ?u觸-þ?î¾}ˆä7?}fÌÖŽ4?RÀËÆjC?dcsߢÌ? -ÏZÁx£?z&X­3àóAGN4FGL J1151.5+5859?͘ä3¾@L>-b8Ú<À9¢àJXçÀ<U¡E@Ý\u éZ?ûY
Ð>?³ ôpTÒ?·9@þÍÐÙ@ÅÈFUNç@OKí"C?ä
¢»Jî¿ßBÌ-jœV¿ÕpàÝûÉ:¿Ý8 z´Q+¿ÙùÄ6%¿ã¸ãÁ…ñÇAGNbll3FGL J1151.4+5858TXS 1148+592?ïÓü_°'?`bœëÓ4/?Qý¬Ï½~6?BµÛ|‡Å?q'dãP8?[µÎQ[æ#?ï³+Q£œä?'Ï=M'ûå?ZOÜВ·x?bn	*©ª?Ö`$?€9½›>{?ïpÕ[ä
?xɅò-B?ië—™¸?e
D´ä?†=°ài)?s֒]b??î\U_?|_Q6bïb?"ãFryÜ?ah	 á‡$?¥&¦£?y±?Ö?Id?%)§'?wÌk@|Z6?gõ‹ý²·?ZãópTŸ?…WÓ»#c$?t·
ß%@·?ïïsüã&?˜=§/£>†?rF¯=ý	?wÕM¾;œß?˜e©­,?"¥ëîm^è?îÎy"Gx˜?'|©ã'‹?|Ã-6N£?|i/Öö´	?ŸNüÌÌ?Œ5ÜRHC³?ì<ª?†?–͐£ ó?•¡>êя?yjO9±?¸ÖÒ]{g?•¿æzìÜíAGN4FGL J1151.6-2115¿Ý:Qàrq@CÀ¹w…r›À:üõÊò×ùÀ<–þï^È@ ~Þ¿¤ó?üáX"Ì?ÌëÔWÜ?»k/ùÂÏ?ñµ¡7Ì¿?ÿ8¤aHÅ¿ïênió9?ïò`ŠÚ9¿àh"¾é_U¿Ñ²ñCú€º¿ä
d½™Óü¿ØhÒý='íAGNbcuNVSS J115140-211345?ïØ®ýÙà?g'ͳ`ÄÙ?: Vÿð€{?/ŽÙ(Á?qþ{'l«I?f,£(£2?ï½¼ŠÏ@?wÜõí'Ö?W¼X…Ý
?_sh³²?{2¤pÎÑ_?qâ_a^œ?ï‡<Xk/?nt¬Qž4?^[ÿ:ùGJ?C5Œy¬‡?Še|>fƒr?luàÙ&}ê?îÅ'äÙ?vh6‡¿ê?i<¨©Œ>?`H·ï8<?ž©k>:Ä?t]BH?ï½/6!q?qþ_ª×!ï?IU>Ló?@ûsÒµÛ?~DÚnÛ³Ð?q
¥Y@³?ïB1†ñÝd?'ŠiU")?iKÖÀl_?sJòOdØw?"TZüú?;ó«pÍ?ï1Ù	­9?}±Ç¢m2?eŒÓ½å¬?S)Aj±?—Dm|·	?{`øÄ~ ?í ;6ŒÙî?ù<Y‡Ì?´ÆÉ­	?u¦i»pG?³‰ˆ,ô?ŽWLu­ëAGN4FGL J1152.1+2837¿Ô%/%͸@S40@9«óÀ;aga8)<À<ć0
‰Ç@!?Žµâ¥?ýÀ(Ê#¥!?ʑ8wß`?W]άÖ?ÁåŠ2ôI@ù
¿cí¿íIn¾¤•÷?됫´NPÆ¿áѲ_c<æ¿áqùAŸÝ€¿¸½=ã^¿ß$ù9{øAGNbllGB6 J1152+2837?ïÑ´@ÊK?'mÿÜ÷kÍ?>™¢»êê?+¾¡è[â?u<\²ŸƒJ?'eð—{µð?ïÕ-C…õ?wE?s·•?A^o®öPÚ?JìýSãJ?s=>‡^?uöPZ¶"?ï[ÚGùW´?#IbÌâG?^ºõH9Õ7?dB]œåÑ?'™´| ?}~Šœ¥Œ?ï–#=¥Z¡?k Sq¿ÿk?Y@Ëî¿j?G€õÍ¢sc?‡O#äßß?kš†Œø$­?ï¢'·Áè?yË¥ð<?PYÆ	;³?CEÄÙ9–?…n¢‡Mò?x¨@S"Á?ï‰zŽÖ5ñ?Ž'û¶=jú?R`…º^G?_(ÕýD.C?‹UK§Zé?Ö|x÷?îº—´è?ƒTÄä‡:?füÛ¯?`‰˜Ìhn–?¢ö>ôÓG?ŒÖEŒöà?í§Û?‡AÝnPWÁ?nr\ï:O?cÂÔu='×?¢µ:yD?‡}§ƒc¸'AGN4FGL J1152.3-0839¿ë'Ò`h(;@I¸ÿ!³®ïÀ91÷ÃœcÀ<¨Ü,¼@ïapˆSK@è#½tj?¯
^\N,?µIȔ.@|Úa
@å،s–?»kÂíC¿å;*®)s—¿åÁ »¿å󾩛¿ê"œý|B¿és$ºÊlAGNfsrq3FGL J1152.3-0841PKS B1149-084?ïåUMuà?wðê´t?BtPTÎ
²?L¢»Ù5õ?f
ž6&ü›?t…†º]%?ïÓm'þ?pó¶0¬,Þ?G&-Ûåx?QŒmô;²?si2)&Ñ?lƒ@‡½S?ï«S0†Û?zïƒ R{?cêEæ4™?q`à\xM?€0­î¢vî?sõ¢ÁÑë?ïè3@ÛMª?Iƒ§»¿©?N_à`V¾?1·G$?£Ù?`LgJ³ µ?Dîk:.!Ã?ïÇç¯É~0?nµ³6héÄ?Rð†'?Diі€¼?wP'ë"{?l=Þk³h?ï!Ûƒã?dÑÐg˜?Z=tUk…?eÕK¹¬˜?ŒoÚªò6³?ŽÔÛo¦&?ïn:á[?ƒ"'-÷£%?k3¿P ´?oA¦¬ê;Ã?«Ay×cR?€9°﷟?ﻢL4zË?i«–æpÀ½?fxƒ9¼'?QúY,Tk?vò™¦\–?dyûLô›ºAGN4FGL J1152.8+3308¿ÈeÇQ…@RÿÀ6âëÀ:œÞÀXÀ<}׺f˜»@§õýȘ@´Å¿'Q§?¾]b wóñ¿½TÂá!Ô¢?þÍðÁ@Ÿ¶2+¡D¿Ô¦"Sß{%¿ìwÅü-ã¿ëÕ9¸ˆr*¿Ò¥ñ7"+¿é(ýOL?³E'Q}¡AGNfsrqB2 1150+33A?ïƳ
Xôc?˜M'4>ƒÆ?PòÐ{Zϼ?V½þ-bþÄ?xiÆÖ[Fn?˜3!ä4m?ïËÌÞ%ËÓ?€2;:åkl?PVL+9?]ö¦üâÌ?vu҆Ÿ?{)!cáQ˜?ï?(E)¼?'V¸¬+?`¿"sý¸.?eچT0™|?`("Ž?'‡L½F=?ïêA'+hä?PÜð-ô;?RpÜÚ¶˜L?Bïè{ì˜?Y°;þ?D"¬&ü<ñ?ïÃÙ´é1?	…£º"/?fiÖµþ?dˏ¾'?sñ]"Œq?z€±§L?ïhœ/¾'?˜v$N¯?j8:£¦Î?‡%öHl‰?URùÖ?'j~eá†?îs'3sÊÓ?™9ÐOF
è?p]®—¼¤}?sÓؒzVã?¦»&òˆE?˜4Œw¤?èGÒ}?}¥¹g\1?{‰GJ¦?ytÕûVÆ?x¶DǛ²?k£ÓÈAGN4FGL J1153.0+8056?ïèfuʖ@Aï îؐÀ:+jК¸À<_ÙSÃÌs@}à}Ù @Zt:dÜ?·hfEÚ*¿¯Œç.¢Õ­?ò×z:XÁb@ꗶ?—›?íº¾?©c¿äÌ°èj¸¿ê8±ø50¿æ¸/â縿ì̼¦äÛ·¿ïÿŸzFAGNfsrqS5 1150+81?ïô­¤k?}:&M?H"'vd³­?q¾ÝÓ_?Em"kïË?h"î؋ú?ïâ‰F)õ?mÓ®ï$d?Bm›¿±¬Æ?RÎÈIHU?hÛR½
c»?gW˜]?úè$?'IËØ0…?cµ«Çé>?pʜHY
â?"$T"Ã%`?~Ñr0n'¿?ïõ
N$Ù²?6ÖSx´Z?B©˜¨ðª;?+s![ó?I!.	×I`?1¥ÎTÞ3?ï÷""JA?J‡Iœäšr?H2V¨¨ó?D.ªZ*?6†¶?ÓÏ?<.²ÇÒ¼?ï¨g™±`?'ÅÈ©Øþ?SGÉøßÌ?`Ï¿ª×,î?ƒ} og¾?€®£ÈàÁ?ï[¿ÔõBë?†]tÅÍÎ?hœÚÊ
?l;âíÀS?'tÞÇ3 ?"!,抎?ïÚV믌?[p ]™ì?aøI=»ÁD?RÎàtˆ¶È?c°Ëî2I?Q±AÍö©AGN4FGL J1153.3-1104¿Ø8‹}³EM@H¤eƒèWmÀ9ð4îõÁÀ<6¶³…Óê@clùþ^?@0>Œ,Ê?·c´Û>˜?²ù¤)ëa?øopJ붝@8ßwŸHÛ¿Ålê¹ò«¿âõ}ðñš¿æt«"­ÿØ¿âvO¿êñxô¿Ù8ÊKéžAGNbcuPKS B1150-108?ïê–9üÑ?hêƒK¾‹?>éðÛdéæ??]Ö¦fšâ?aŒ£ŒÃ?er1ÊJ5?ïãUð"@?oYy_'±Ö?7n+'%…‡?EEigU"Œ?i½o	¾?lu"‰åŽ?ïµxâؼ?uߤïyÒ)?W\štZÑÐ?DۀâfQ?lhHі?uÔ¤RG?ïò?ŠÚd?<W€°Ö:?1Ɠ…9"?WÀ©âCÙ?WEI3›P?:Ñ!‡wR"?ïÜ¢ä¾S?g°Jͼ‰?JÛå¾)š?>®Ðkí£ý?mGcÑìˆ]?dòj–ÐÕ.?ï ©‡®‹?‡ðÁ7‡©?N);aŒQ?[iÃqU­?…ó
'7ý?†°1áWE?ïuƒ¤(­?'Ø?‡?c¦èa¨¼w?XZ¨:_b?µ\Íô/¶?€Öø®À7?ïÖp>xØü?]5¨³.í\?KïÑÞÄ´O?7LáŠ+{i?qIæ˜ÅÈ?ZµôÆtnÁAGN4FGL J1153.4+4931?à0£«>î@P?W}•WÀ8Þê'ò#À<AÌN!Ì@˜ üö@ŽŠ#Û?¢Ã^äçˬ?£ãñ¬€&+?þäԕîê.@Hm²(‡¿Öыؾ¿äÔú˜¸¿å‹MpÌö¿ãs>í¿í=HËJ썿ß9Ü>YØAGNFSRQ3FGL J1153.4+49324C +49.22?ïçïœÛñ?[s@bÂ?@f^[mR]?13ñY4q?cöÌ`zm÷?YWAÌaÄ?ï׎Nâ¼"?q¼ÌY¡eM?BÛ¨ÿÅ—?P&	]5gÙ?qÝc\–ì?ocwûb'?ï:²í8ä3?"ŝޖ±"?kï€úþ3?x°p %›º?•+²5qÑÔ?"©¢c2M‡?ïÿ î¦Ö?hßA+­?oRF'än>õ.AÔs"?*‡ˆgá?_uUêl?ïËâ†iÞb?upuXӝû?L®?ÎhâV?@nyÔGzä?vxô»¯À6?t•Ãæ'"Y?kÍ¿¢?V¸^ÛÌ}?PkmjžOÓ?^3‰{!h?‰Ä·bSów?Œp*1TN?îÎØÄìrs?›JCžyøö?k¾7²¿?r—þ½Jâ?¡VD+4(?š+]̚ë?ïýžŽa?)ãBô^µ?MÙ%¬?zr‡BÇ?'pœˆaü? ÌÊS4Ø<AGN4FGL J1153.6-2553¿Üƒ+…%*@A–ÃÉîËûÀ:…wqP¥4À<mgZ',–@ BP¾ßNZ?ü5 *­R´?Ãõ]$H^¾?ÆÙHƘUL@1æaÉH´@Z9è4¿ïñ¸ðiŠ?ïE®*JVe?®@ê</—Y¿ß)¦W>
¿áÊ°]*}'¿ãž™]´'AGNbcu3FGL J1153.7-2555NVSS J115338-255412?ïÞ´®rïŒ?y¤ãx?[?©à¤ö
?cÑe!"?c«|Ðøò?k2‹a€J?ïÒi$Âé/?tÿVz•ä?Qú»qÔ?Z¾SžËÐ(?rL¾Ê€—??o\Õrp‰?tio–?|øÔì>¢?Y÷L •'ï?_M'³½ x?"^ùXp­[?{z>Õ=
?ï1²]œ?mޖ'çõx?s°øâP«ã?S])9~ã ?"ÛQn{?k'1E¾?ïÓöŽßxÃ?jÁwR>¶?ZQðû´½?P+Ÿ ¸¸?nàxy"ƒ?g4ˆªa1?ïŠÉ´¶ÍÔ?ˆSå™óÍ?]êªÃå'?f¤ùf	Q"?‰R¶ÖO?"õ fÎ|a?ïa"ŽçÜ??ƒÐ¨ËMP?e¯{oCÑ?eó¹› ¾ ?'Šs>™¡?'" ËàfN?î3¤7µ×p?ˆ€´ïÕ?Ü@dÌkÕ?m›Aäú´?¨N¬gOæ	?†~Ç2
AGN4FGL J1153.7+3822¿ï©Ô
•@R`{_ïJÀ;i°Œû%¦À<ç¥'lU"@ ¨RÑ^,?þ­é—Þ®w?É´—L?yœèƒŒ'ô?µm‰_(žI@vJ_É¿ï7óâ:rB¿ÊRŒ)nŽS¿Ð¢0aFÁÛ¿è'Ø¥H#…?Ã^jÄoF¿áPå*'¤AGNbllB3 1151+386?ï»×AÎ_'?r…KíµîÃ?F"v¼—'?:O‰IK?CÐ6©'^?q¢bÀêkn?ïÁtÒÃdw?{Ð~bÿz.?LîmF¥²?U¹2ù=ú?{§Èåñ8Í?xÒì vˆk?ï ¦à÷I?ˆQ¨	&?j1Q©u§?qiٙmá?šõÀêt>?‡nA7i	?ï¾ÿ(áíé?d^ŸxxÞ?=¤O(k?0úÑ#0ú?~®ù÷¯?dp5îáŒ?ïy&gGâÃ?†a)ôAÇ?TûðÎJ?IÅ.©s}?3E§©ý•?…LøC¹ª?ï]|C…?•;üK
Ç?WYÔõ°ß?g]Â)º÷S?'Úæ:èü\?"â|y‡²:?îN£n¯‹?"ǹ¶œ>?pá>•Ý7?q*3"³Ôú?¨ù¡B	®¸?'xØÞòÌã?ï}]x×?†µñ"‹A?SÙ¾\ýs?P:3¶B?œ2¸eÁã«?†%^;þšAGN4FGL J1154.0-0010¿ìzìÅ»‹‡@M³þCg]ÝÀ:ÄÜ=ƒÀ<:贉ßè@ ¡Øñd?û¨À˜áãµ?¾(²?œ'à?®1´%Ÿ!?óêIš}Å(@ÉÌJØÁ?ï÷±j8X?¥^w.µ ¿ã?@óVµ¿ÔEO_¹£û¿ÉÁJ£g†¿æ-h¹&ý›AGNbll3FGL J1154.2-00101RXS J115404.9-001008?度ªuÆ?zÉ%KF?QüE­S ¿?I¸ª1cü?ƒ ®›Õ¥?y'•«°jê?ïÜõg±Ñ/?pmL+b?@ËF¦î?JIb.Ÿy?n×Ɛž¤k?l¼." ?ï9L‡˜V?Ž³pØË­?]á¸@Ÿ"?jÜ¡º#·?–øSƒø­?Ç-¯dƒ?ï2!àFô~?r6>dAƒ?fì¨)hOé?K%@²Ð€?–Þ.îÙW?q½NÉ"<?ïIjl&ç?»Í,5k†?bª{êC'?Zå,šýš?"}cv	¬?Ðý·en?ï…Ô¬Ù×?m'Âñ	v?W QÒ¯1«?iu$T~›?‹–Ê'œº?‰<‰qy-?îUŒN'o?ÇÜ"Ff?eŒ¶P™?hå1ôÌ÷'?©N9Î÷­?höÞÀ?íÈÉ6⌟?:™ð0É?}3"h
ƒ?i¬ªòF?¯ÍCáÐA?h"ªOâAGN4FGL J1154.0+4037¿îžµ
y¡h@RؤTÞÀ:KO7u¸À<Kžd¶@ŽeÖÉzÞ@¡·D¥?»©¥Ö=ä½?žçÚø½7?âÙV}»Â@
€#½Ÿ]S?ï¹OýnUH¿¨³oX¨bµ¿áŒÈ›䟿á4Âkðê¿å:c©Ä\¿ÔdfÜØÞ~AGNfsrq3FGL J1153.4+4033B3 1151+408?ïó+ó<¼ä?FC½‹"H?1ïi~Dg? Biõpáá?U,>ñ±x?D–QšÓ¢?ïÜ_K÷p?qd¡ÞÃ4•?B'\ìZÍ÷?M9S†øö?nü]¢â1}?nláG¸?ïÃØ€«?e
J#Â)i?S\íËæ ?TÒõLÊ`?y¡X"¾€ë?a#r¤Kõ?﷖©Ç†‰?^æcÅ?h"ü&‹?I¥;™mw?wê­-ë?YAp^?ïéØÄ°QJ?R-1ž™??èAƒ_i?.S!LVM?b*3©ï¦?P29qn<³?ï'óJÃ{H?ˆôÎ
Éäc?S¯ïÆõ»å?_
¸ö˜+'?‰
/Z¹ô~?†³Ý÷ôA&?ï›|Ú_÷%?q¹løm»Í?[Àš¿X?SÁïå?…¨ÉYÈÏ?o¥xQ¢Ãe?ï-øhSræ?{Û-,ÇÕà?€ÀJAD~l?e•<ôò?¬?'àÍÝ.sû?w9€Ògß?AGN4FGL J1154.0+6018¿î[" Íf6@K³û?¦ÞüÀ:Ý]=ȸÀ<FDw(UŠ@ý¤)j‡ˆ@j$aY?¸ÅxqÖ²?ÎÐd¾›‡@AÀ6@ÓÖ;‹qc?ÙêY¥Ã£¿âRƒÅò½ø¿é³ß¿ëÔ9~§¿ïþ{ ۑ?ïêӝ÷LRAGNfsrq3FGL J1154.3+6023RX J1154.0+6022?ïÒê"Ô€?–ëTpqa?q,ß)	?'LlŸxq?Wã´H[3?x)ixlj?ïj<°ë#?šM.E³t~?w嘞è{?"¬_=)
£?‰~¸JWê?…V‡oLHk?îÃäÅó—?•@¾5N?–H–Žûš?'­x"ðS?':Ðùfº?‡'Ã`Õg?禍§»?g´"ö¯'U?uwlxB>»?]Â)
»?u¿ƒÍMOè?_¬ØÌÆ}ä?ï¨yñ³Œ	?'É'2‡±¤?Åó%¼Q#?€<&ðÎï?`nA©$v?dœÖ<©T?î}´?|¤?­3#•qÆá?†q÷ív‹Y?›t¦A´ž?¢ˆ>-…ç?¢ÞbßZ?í»UYVf?¡Åbc6+?¤òWWZ?œ%ÏÖ2è?ž±$$ÍiÖ?'«$£¦ÍZ?î;2Ív"°?•ôW,?Ÿl&X)?ŽTiK¹Šý?™":#÷²Ó?‡£/'à_AGN4FGL J1154.1-3243?ïeA°»@<Ÿ¡<%J<À9Tm'LžÀ;ñ´#ìn@"XWÚÝ\?þðCå2`?®wE0áŸB?¾ÁÀ	@t\!iT@
¨!"Šé?ð¿ÜÉ/^giq¿áª¿†¾ ¿ÙœF‡£Íпç¨S;wG¿í™šùdAGNbll3FGL J1154.0-3243PKS 1151-324?ïy8]"…´?¾!œ%Å!?Åþ"…?¾&Ê«E¤¶?Q'Êü€?QÆ ßAš?﬐ÚáÁ?€×\_1×Ô?d yQ5‹Ø?p´4"çú?§U愸p?w‡ª¿=æh?ïNøÉTó!?ŽxÜß%?t^»\lÿf?}|Y@…Г?'	7ûÞ¡û?‰äÎÝs8?ïRžf²?v"ZÀçL?ƒ`.Å®?aۉíká?–%¬¤Š?q¿•gì?ïÇZÜ^T
?¢3õŒ?p'·Áç…?¢'áø+k?hsþvàSŠ?d¼p/é?ïÛà]o¿?œô͒‡'?{x'Ĉ—?‡¶éÆÄò?—†_†÷v1?"®Mó¸Oæ?ï"/M>?'Ðçází?€›½•â&ê?…s¦FÏgõ?"¿»TDôÓ?£&vŒa?íÁ"¨²¢e?ŽÈ}¿e	?•aûÊE›Ü?{њø£o"?©<׍û=¿?ŠK1!x/CAGN4FGL J1155.5-3418?â»>ÛïÔ@;%ðÃL‹À:=Áz‰3À<O»S'ÅA@ ³‹WŒƒÜ?ûъŸb0?¿ 8Åxr?³yx€´	K?öœÜ_@Ÿ1czN?ïþ»ýq°G¿ç$O€íl¿Ó¼GÃe¿Ð\¢õ¸Ô¿äbÐzw¿·Bï=åé©AGNbll3FGL J1155.4-3417NVSS J115520-341718?ïËÁÁn?sg
Éuä??R­:Ïùl?0à*Ôôÿ?x*JIVãu?rÌðUâcy?ïËâäçß?vzCñ"?NCy¨"[?UÁ À˜¢«?vF8únX?r>QŽƒâ?ïc`.S?…0 +…Ê?Z•>ãþ?Vý¹?'ꜫЙ?"µßV"tƒ?ïš.XÈ?pyÆ0ñ?p;'úOÎ?LÖù:Ág?˜-¨Ð[\#?nŽÌ6Óêa?ï¡M;-cÍ?"×ñèŽj?JÁµá~ÐÛ?>¶Š$-Ž?†•ÐW	?"}{þ>Žû?ï'ç'ø?ˆ515
E;?^4´¬­c?f¤÷Ym?‹»>]rr?…+•>œò	?îÛt°ß?'q7µ)ì?cd`µË÷?a*}é %Ë?¡¦ë•$?'£AÊ\?íšÒ«ÖT'?‰âŸëïÝ?ƒM'F!—?gkÿg\»,?°¿¸zúÉ?ˆ,ǽ#oAGN4FGL J1155.6-6547¿×8çÛ¤ŠÀR¶ä-;¢À9Ö%Ü2›^À;;u –
@Åv¼ƒ)@ê໗?ΛraÇEN?Õ« ,ZÒ@	WQ:…7?ôxƒ<
d?ïç)€=Ó¿áD7%?U¿é¤óÕORN¿ë¸ðvö£¿ïýwקò?˜cï=ºöŒAGNbcuWISEA J115414.97-654215.0?ã÷ìøޛ?Æ¢¨‰Õ	?¬u'*?®ÐFþçÞ?Ԁ#sDÊ?Å
•™·?Õ.šÃÌYF?Æõ- f?¸¢%'"q?¶Eý÷»Y?âTmù`\??Ã]Ê°Òþ?à—öQ#?³˜ÙÆ©t?²ÏBâ—~%?õé)8ƒ`?Û4ÿZW~0?²²k|÷?糜¾ÖÚ?—k30\Í?Ðý·º°¯O?¡äm†Îã>?â—7;wò¢?£Îc'$%?ÙÅä Óõ‹?Å®D¤Ê¥?ÁÏñYôèö?½{ÍMG¨Ø?ÝR"²1•ú?ÆÖ
ñ¸È?¹Ž×°?´åî‰"J?ÀZ…Ýz!?¾qÿKÐ
?èƬ­{+x?À5Êt$a?Ðô/íƒ{ ?± ç_Õ?¼ÎÆÍ~e?¦¨p®Ä?ãì0'BÃ?´22â®Ë?¢ ÞïOˆÈ?'•wÕà?Ôa^iÃ?¯OA'¹?äÐð`®I2?¯Ò­äMIXED4FGL J1155.8+6137¿äbÂ0Là@K!ýÞ½À;˜Mà]£À=™0¾
í@!
øæ0K!?úèÎör¸"?жÙÛÓûÀ?ŵ¡bê"?ö¢XOLnn@)¬'½¨?í#·•-#O¿æÈóĈZ­¿æ×z:XÁb?»òð"wÍ¿ÝÉ/‰Z‡5¿ä,\\×qAGNbll3FGL J1155.9+6136SDSS J115548.40+613553.8?ïà@m6ñ?^b‹u?F¥DìAó?7?o?|l=?jAëÉÆj?ZݖiP‹?ï'ÅƉ?ƒ°HVãÀõ?`ޝÊ͹r?a)eoC¦?‡WšOI?ˆƒ¾ ?ï_8Ë´°?>ÍDê´J?f,á~tú?hˆ{"ʚ?'Sb¯uïˆ?š«¢¥3?ï[–ã '¡?rëAçù:?o6)‡w9?X©6&!Ç?¦^di€?q£~âk•?ï¾Ö\ E?s!–Ïw
‰?TÍsK^E®?O9"Q֘?{Ê8FX?p³UµòžK?îóü6G?›Q¸ç{²?pM%O(\ð?xqYõƒÎ?Œ"%ûâñ?˜y rÿ6?î×q'	–=?‰
¥Bå?oߚ̠à;?nÐø9¼×
? Šî/Bï±?†ë!À|ÙÜ?íÑÌ¡Œ_Ó?'þªžeä?†Eµè>?zåTí'÷?­QÈ¢*=¿?'vB'1AGN4FGL J1156.6+0640¿âp;mOŸâ@PpmH÷QÀ;eEñ{ؾÀ<¾Lj;Ýý@HãHº.@q<î×í?Ø
PJ›.Å?Ó5ÂÅ+?õã]gº#}@
Ì3j¾9¿ïõð¢i÷À?ïö$´ë.¸¿Ñ·	ìèÌ¿å
ö~!)¿ïñÖ¤¿î×oZµAGNbcuTXS 1154+069?ïÞ]ô°t/?da<âZ½?QŽo™"Øñ?H3|ߟ?hÚÓÁú´?`5Øä?ïÑ^›'Ž?tËCŒ:?JÆ
Xý˜?T-\Ž//ÿ?s÷ðÂkd?q?ìÿóà?î¬$l'ˆ?•Z#DÐ)ÿ?Œ5d±rÃ?ˆ•êîâ&?œ`À"Ì?t™dR€z?st½b»?cOÛ?g¯w×c?OÉηæ?~€ŸÄ¡E?^§9›$Y·?ï²FNÌtk?€e;Öÿâ?cÕjÞKÌp?[ú#»?|ò#4î¸E?}‹>ï R™?ïyÌäc†&?ìfÕ}ô˜?_¹iÐùŒ.?kp
ÎYž?•™®&õ?‹¹ÀŠÝË?î)f—Ó_¨?™ÅΗ,uã?¤q?Œ`J…™¹?¥\ÄK$ê¼?"Ä,y·zK?ïRý˜>=?~Bãy"p?oxaDLc?cÁˆÕ2î0?'¾]îÿ™×?{_MTó3AGN4FGL J1156.6-2248¿äˆàÜ@C+8`™ËÀ:mAaÊsÀ<_†z%@ð\ñržƒ?ÿ"òXwZ?ÜW¹û8ñ?ÄǏ¡F@"à¹(«@¹
¨4<¿ïÜl²°Â?ïÞÁÉ'¿Þ¢T~1‰:¿á[¹.׿ۢÉä:&¿èG犾4"AGNbll3FGL J1156.7-2250NVSS J115633-225004?ï·§'^Q?mqæë
¬õ?c!	éüq?WR؀ÞW?z›²"ÿjÎ?gè#Œx?ﺙŸßêó?|X‰,Y½E?[׶ÊQÔP?bæýø•}?{½B"=K?t¬ìÁ	¤1?ï‰ÆKd"?lÌj(Ö?`÷ºk15‡?NyŠ
këY?‰P~{8¹
?i
K Bý??ü·?y·®F¾?ˆFŒTÆ?h\Å} ?¡b{3¥!?xÂ
I?ïv€<Þ*?€ÃJ&C¨x?wŸ…'™è?nS
cB‡?†.w;ê ?wøÞÁ‰¸?ï3™ûÇ¿¥?"†³Ö	K(?nñŠD¸"?u–ãöxÜz?•®As_@?'¢Ù"!U?îÿ´•[?‡>Kj•?q'UµïÀ?dʉû½¸I?›·´.<Ë°?"Êf|G	?ìMýƒܐ?"|´k
?›o‰è±
Î?"«èFgýÇ?¶´1ojšH?'…[ºn"AGN4FGL J1158.5+4824?é蕼P@P—BÃÉîÌÀ:3(¦É-À<…bÎ+qž@iXûÓö@g6:N°g?¸bÓ3ïÕ? ®Ý½NÄM?âÆ8Éu)x@ O¼€ÏH?Ý	ß<fÏ¿äŠLŠN¿åµ‡k™¬¿çµ½A›"¿èWõ¹€¿Ýõy(àÉÚAGNfsrqGB1 1155+486?ïù"æxçÀ?=\+]Ÿ»8?%€§¿Ì%W?Æÿz~"ù?DL;'eÿ?:ù¿vÞf?ïæ"Ÿü#?iAÞ2*±?5Ò²?%"¨?CÏö£H 9?g-%Jâ¶?fg†—I`?ï½çhsJ¿?g'"Fá?Tœ	=ÇÝä?S–"Z§õ2?{åIgu?di‰Ùú‡?ïøq»Pšï?0"ª°à`'?1‰—.Û?Ïþ€,bY?Eq"ÚtE?+¿ß9ûý?ïô¡AÁZ?J·".«?2ŸÅDõÍú?!Í5í3Ø?Rø§~"?H¯ 1	"?ï¢ÉœÒÅF?…ôÇw)V?J®²)?VìÎþ]ò?…­G.9d«?"tÃz)n?ïuh‹Éf*?»S·?aþ¡˜Ó8?TàÆ4bœ?Ž&4Îçú¾?€g0‹šË?ïê9þ£³?O‹ã	7~Í?IÖÅÁÝR?6r¦‹¸Å?^  g÷²•?J.g]6ÌAGN4FGL J1158.9+0818¿ïê=9á@PܵÜÆ?À;ˆCaÀ<§óv"Á›@ 6°Ë9yÉ?ý[ÛÈé~?Ê@åxjIö?¶ºùw]?î<G
ۊÖ?ÿj?›Ü??ï‰þ›üË¿íP_ÿD^¿ÃEyÇAGž¿ÚÚ¨!ò™¿ä‹ÂÁ[)œ¿Õl—£TYAGNbcu3FGL J1158.9+0818RX J1158.8+0819?¶»z?md™Ð~?EKFx3?:˜:)þ	Ù?…íd[šª?~þÊҟë/?ï[¥û|¸?öþÅe?nÓEeþu0?sª¼E,è;?°×èx"©?‹÷xý)Ò?ïVMC³<?ŠÒŸ©6ó?a^ÔCàÔ?aÖÎ	¹i?"»Ðmn­?€øþƧiE?îUG‡Jƒÿ?~Á@zå ?ºLãw¤ø?cm4L&	?¦<ôU'|Ì?}p綏?ï:caµbß?"â%W$?RƯ€yu¬?Eä†ÇÂB?—‡(ÉdòÐ?"Û…Ð}Ô?îj$mƒÍ?¦îoÆÍ´r?y4B§jb?€ûÖ»¤?¦9hz›Z?¥›:r[€ô?î¸û½·A[?4ëçf£o?j}ù.ò]2?m[¾Žï?¢ÈdŽC%ú?ŽPNA2y?ëF`×}¢?œË'<3K­?'"¢,óЈ?}dªa]S?À•6•›ç?›–"öY‡AGN4FGL J1159.0+0939?ӓ|DÛ7…@Q&8ÅCÀ9¼b †ˆEÀ<H}'ÒÕû@B™³šÌ @¥?|í'h?³Î#Žû[?°ý<aNÏ?ü«ÓXI@7}	Àóü¿àD'❪?ÓÚL|°TÇ¿ãU38;°°¿Þs]$žDú¿åÄz¿ç=W^‹¦'AGNbll3FGL J1158.8+0941GB6 J1158+0937?ïôˆ˜·¿?Xαí¼?1%Ý^…S?2J=…•?R·w†ºeâ?Tã0õ?ïØüÃ>a?pؾfTb?DžÇqârS?O÷íûX{?pîǪ?l´ö{TZ?ïËLp?\ßY 'ü³?QïçÐO‹s?F
{¬´TŒ?v_Ä[²?V~>ÛÆ,z?ïÕRϨÖ?P‰ð\³…	?^ŸH"à"??8@©Mè?k]£cªw?H¶±¸?ïï`ByŸ?M8N™¡Â?;)BZp@?*ð;Gò?Zu+ë‰-?IŸKL/K?ïÕ€¥Ú?†ˆÖï3«³?V¤º ã?aéÝqe>?‰¶‰=5S?"j"–sI?ï¨áY»vþ?sJÜ/ˆß-?Zš¸êvÃ?Zwù-úIh?'tR}rfæ?qAËÞ¯ˆ!?ïš‹±µ«?l®(£^}³?r²Š|Dó?[Ág?œÐ?€&Z]Ĝ?d¦ièÒ>AGN4FGL J1159.2-2227¿®Ì,p¤Âg@CjmŒ?À9/v>J¾jÀ;ÃQvëè@–Ÿ¤J¢'@Þ¥rðR?¶fŽ_0½?ÂKD÷Ö»¹@€	ö#l@3M™Þ?׀ÒbãÏô¿ã¶"v¿æ–îÄnYz¿åX³ UöW¿ênjЛ¿ïÿ~€8Ÿ"AGNbcu3FGL J1159.3-2226PKS 1156-221?ïÞĘ9¶õ?`âhI{X?RÖrvjĈ?Ijg¢Ä&Ñ?gÐ.ji2?Z$L;öõ?ï×¢7ð(¿?pÁñìùá?HV0Éh$L?Rg‡•äl÷?q$	®¿?jn;3/n?ï0sv?"³Îáëf?pòÝÖ~?uîl(úúw?ˆ0ÿ£Ð'?€DÖ¥9õ?ï¯Lغ…'?a®7ß'?bÆJäj!V?B"OmÄ&u?~ön/Ø:·?`0çS3ÍC?ï«õ§À"?vËûžuç-?k¿
Ö>ƒÓ?b]ÅÔÈ0;?|%¦½Ïoô?rÓôÛÊñŸ?ïs(݀	Œ?¾WrðÆ?`}DD¼W?k…[Ïž¸?w'h	ð?ŒÑ¦¦G|ì?ï*G r]¸?7=…¦Ûg?z«èîìÞ?}B]6ت_?"!¯#ÚÖ?‡ú_–¹Kƒ?ï5¨®_y?'%
$•çV?"~Ýdh?fe‹­Å6?–Ы*oþ?€çß÷C½AGN4FGL J1159.3-2142¿Ñi©"¸@CÈú?̞ªÀ8ÞqÍ¢µ¢À;¡"ØaV@¸‹Í(<@çüÓû•?ªD?è<.?À·—FBÐ@á¼ýKð™@3®~Øù¿ÛTbWä¿âûîç´°¿å` ‰wãf¿ç9Â,_Ú¿éá1ޟ](¿ïþžÖð<>AGNfsrq3FGL J1159.2-2141PMN J1159-2142?ïÐä|Ÿks?•ó…¿æ>?d2"Nɋ(?r ãQ«é²?jèð	‹ñ›?p×c©à?ï™=¤Xíà?ƒ.åcL ¯?fØ` ?o(‹óm?ƒú~Âmð>?{ö:ÍhN?ï¤O«—{?€ìò¦·ú'?häê˜ÃR?r¥ØcND	?€²Ú¢Q%?{Ùdò©ó?îö'älóì?x)îäë?""—'ˆw@?dìÆw&1Ø?–ð·¥­ªò?sàèn%?ïŒt,f?¿
x"Š?pRy•?eŽK,X3'?"îyž;9É?Ž¬º&î1?àù?¥îÅäüè?€%|Ø
?…6ë6†?¡ýÀx•7ì?£œcб.?ïuêÛß?Šf>08î8?uÂwŒ"Ñ?€¼Up1…?‡¤
4Çt?ƒ<µN<4J?ìﱌ.L?—OÚc[P?Ÿ•Í¾+¢°?"ÎkЌ²?°ä¤ó?'±¤1Y1AGN4FGL J1159.5+2914¿³ qÙú¶@S˜	¿œb¢À6Ù¾´Ü?À;tR¸3¹@
ÍËzgO@ӎ¢Å'F?‰ÕQðQ{?¯óæÖ¹5@"2~À¨@!æƒ.Äd¿Á8'Ù÷¿ß#½ßÉÿ"¿ã¤Û·K[H¿âóύd¿æT+
oÆ¿ç¶é¡éÜAGNfsrq3FGL J1159.5+2914Ton 599?î$Žú6ñ?Æ?VÜI†K?b*[ï¥õ?w´Y\"_Ü?¬"PÈPƒ?Æ*ç¦(."?ïŒVPªÎ†?iË&­´q?e­kHN~?zøajD¶?‡ý	rÉ?Šúª·–]9?ï‹B¿Já®?Žàà='?påâ¨ZH?OãÜ[}?"¼^،ûO?‰ÀšLb}O?ïúŠ·BeÅ?5ðX¸T?!&ÍÉbd?JØ…N§?A‹ž7\?21P^¼?ï¾_ÞÚ7ç?owédíÉ?E´­mR÷?Aa¾Z=6X?~zÍ>Z?~¾¿È?îü×ôôP?¥Ä¢áÖî?r	œ·2h&?ƒ¨äM…e?›âš+ŸG?¤Ißö^ç?ïrª×Q?'—)P& 5?p¸ƒh¤Š?}rÞ]Z±w?Šù…ƒ¹¾?0%GôF ?ïô æÕaœ?PˀZzI?0/C)?7?-<v™?S²mºëfR?N®Ëž¬ÛAGN4FGL J1159.5-0723¿³
m(†ã³@J¢qÿ÷œ"À:&Nɑ®êÀ<M@± ÷@¬úv~6'?üæ/Äé©|?ÆÉGÝc?ÅڿԖÆ@ÖÓßÅp@ò´/œû¤¿ïÿ틉5ž?ïüî×컿Þ7Ó@"TŽ¿ØoE2980¿ÚMâa®z¿íŒ_¿ƒ8.AGNbll3FGL J1159.6-0723PMN J1159-0723?ïéS,ð|?Vrk~öÁ?HW"ïw?AŽ$¤ý?`¦ý–Q½?Q/Lüähß?ïΖZÙH?tè¼Ï(·?QOžCç|L?W'™#ZS°?ta«›ý?p|—Ö¤©?À¡VŽ?zåpö¢à?\uOYðG?_qύáe?†&؀?yaÇò"ÁÔ?ï8¬êYO¨?obeÂPîÂ?y£wÛX&Å?X:»üè@?'"¼ø_?jЌVo`?ïÖí:^(]?dHdû†¹b?\l½ñzD¬?PýÆ9Èð?jÜf×Õ0u?^a""uf?ïtÕ*¥@?‹Š—è®?bÙ;=>_?i×unN?Žf72J?‡¤8õc·?ïJrõ~`?†úó<'lŽ?f@V†›Ld?hÔþGö'?"é–‡ˆ}?…DüØYþ?îG+ŽµK7?†Ò‹ï2¤?ˆÍÿËÔ^¤?qm€þ=$?¥YÇ%%Ðà?"`®SØtÂAGN4FGL J1200.2+0201¿ÄDkeâó@O–#ûÀ:(*ùÀ<nΠâc7@Ý0õkL@Cx$Õ?½Æ'ÊBXë?½Àdß}©y@jä°a @\wûT¿âõõ»Ÿí¿Ý­† J¿á€>´pµu¿ÛYÄAê¿åSP¦^N¿æd¶}Õî´AGNbcu3FGL J1200.4+020287GB 115739.6+021927?ïö³óâæ??;SâË|ó?-œ‡†§Ê?›gaUü?MÉšüT?7#%5jæ?ïÝõv(|?pNîë?CNþUÍT´?NŒ§¾^HŠ?m6ÉüÉûÈ?kMo/ÉØb?ïÌ.£Λ?`Äë)ø­–?QM:}w͉?Sw2€n?u•_ìXg"?XÅtù-&J?ïÍ×cºÌ?QWVɨd"?W}ÉFìâ?5?Eà(?s±´â°é?O–PŒŸ(O?ïð<Ô5'?J›~HÞdb?;u‰ïÆÒö?(TJîsӊ?Y#»ÀcÊ?F̈Ÿ"[?ïžÇì=Uv?"ßCJl/µ?RcoýC+1?^ÃÚhÌ\6?†—x{?'ôA÷ïTÕ?ï¬b»ø-?j¢"ç¥?WXŽ'¤Æ?DqÜ	N?üh0–üÖ?gäH#»2$?ïx÷˜8­?q^u¢?lÌkŽ{{Ê?QñRàT?Š¬ç.kÛî?oE[2wAGN4FGL J1200.6+1229¿êÆn( @QÉD=F²lÀ:^4Òo£ýÀ<v†oj@÷÷ÔãF·@"Í–&?Àíá\Ÿ?¼¥Ú5@)?ùý ª/@
|÷ÔÃ?í•÷ƒY¼4¿äy'"¿å79ó@ÔÜ¿åÒÑɋпå\ÏAS¿ïÿLa¢—AGNbll3FGL J1200.8+1228GB6 J1200+1230?ïë˜2
q?UäÊlº±I?9ˆ{36ÉØ?&üx¹:€°?a6¾¡ôƒ‹?T³'c–?ï·Ð†µ?s>Ñ}+?IÚK9Ïqî?Q¦kô½1?u€Î¿`F?pkèO;?ïÂø"zgi?`DtýĘ¡?Sr*^W_?=]Ò÷Vî?y§80¥'®?\î*%Ԍ?ï!‰N?c-ˆÃ@X¡?sž$HTǞ?T2ïŸjS?'(‹"ŠI?^p']yœ;?ïÐK¼í>?hÂGnn¿œ?Kºíxk u?<F…c¨ì»?tbÄpéU?g6SýÄÔ?ïo¨}sYz?<žÁ̓—?_`@–¢á?eñå½3ÿ˜?ìLú¢?Šeǔ…†Þ?ïíÕtÖ?t‡J³ª—?`Tå;ü?W°‰…Z^z?‡ê¾-Ý¡?r àœv¼u?î¡åó0Ü
?"bXÿrz?–Ñý´l?t芴c*?œ÷ؗšá¤?¦|³WAGN4FGL J1200.7+2008¿ê¸ò%ÂÝ@Siì,äeÀ:´Ç‰¤À<l´ˆ2i	@Yï`÷'@âÿœ,ñÑ?·ƒÀë?©Ýì@Õæ?ð ó*.§³@	å·Îí?Ên¸ÅXå¿å­U¾xv3¿ç'ù¾ÈR?¿âÛ._ƒô¿ïþ|§ñK1?ïÚ¡–'õAGNbcu3FGL J1200.9+2010TXS 1158+204?ïä~ªTý³?sµ*ë Tö?Kzoÿ"lˆ?Q–eš' ?d¢¹œÒÛ?s!˾ò$
?ïº;ä •?'eµÏ¢Åˆ?YNßó?m¼þ1?|l¦h'eX?y´´—"¹7?9p}Û?}‰nÜ>Î?qF›5Ì"×?yñ¼mFñ?}[H/"b?n¿¨P.9?ïÍXžUt?[ÞՐNB?f¡4`äU,?P(FóöÓ?l¶'AÖñ?Q{ºúÕH?ïÓ¡t­?n—‡jÊӓ?`¨a*¸Ë?U¦DÆ|?lYºO×a±?iÞ©(
ë«?ï;
&aÇ?štځó?h9µ—ŸÃþ?zgò²X?•–‡ªÿ~˜?˜‰ý{]?ïVÖ7ÑõÎ?‡©¢s{÷?wª*Øf?€Œ"`R¥?Žu\Ÿÿiv?$ó¸ª?ïJ™'ù?€5Rž8´Ú?"ĸfðA?s:z)½?ˆ•¹Ov?t±µ,zAGN4FGL J1200.8-1429¿ã —±{ÒM@GMØ@žUÁÀ:é'm{.À<vRNmS@ VÀ"Ûë?þöíï/Î?Ë«¾à%??¸·²3nlo?ìç¬sßÌ@CIËûìu?Àw¿ïçågÎE?îYœô—ìñ¿äˆ-@U¿¿×vÝâžÆ)¿à¹Ö?è"iAGNbcu3FGL J1200.9-1432NVSS J120055-143040?!řõ?‰~|7r?EÚ+¬…åº?4=±ï0g?Š:ÍOÔ?‰j‹É~7?ï·ßŠçá?°«,ÏÃ?Ss~–¢³
?d6 õÚ<k?3•­ '?}@b^ځò?ï?áêÆ?‡O
‰ƒ½]?[âF†¢?O1\ðL'ÿ?–Ež^"#Ó?‡
©w7bû?ï$JyÃ1æ?{,vvðõf?V\•¡&š?LxoƖ?šçtgÕ?z£‰{F¤?îéo˜\©?"í7ýý"@?Tx³šŸ?TyÀXȵ? ÈÚ¸"qò?"ÏÀø!G?ï$Q*9S?ž³jÁŽ?aÇVúæK0?p™ui?™<ã{´0?œˆIŒ§G÷?îCÑ©'$?—yš·%Í?d×9¹'cì?Y!c½•¨m?ªu|JQ¨?—¡>ÞÊí?íÛ	íÀ?™Õìè{í?dºMõP|?`Ò&ƒmwn?²kTÿw9?™€Ý©÷‡LAGN4FGL J1201.1-0332¿ïwO'þ@L'"¦óõÀ;Ô/—@À<nê™fn@Hÿ¥è?þ­[î=_Ý?̇'™£?ÆÂáfŒÑà?ý¯3^Ò@ Ü2ÆQ¿ïÿÀà/€ ?î.-À,«Z?ìNÛ?JB¿Þ…pí¨åg¿çvFŸ¿à)¥÷ÞÉAGNbcuNVSS J120111-033219?ïÇWӄ)£?wñΆHƒ?W?°Ò¥Œ?TÛÕ*u¾®?v"*=¶"å?t'ç~j›U?'¥?‰ÁmòA"ƒ?k¿â'?t®Ao¬£?…aqkñ?àn4?ïBtïÜ?†íûÛ(]?ià=Ez³?i/V»hÃX?"uu\[ ?†S'"¿?îm‡#5\?ŒEðqä?Šˆé—4™Î?€+±<V%.?¢…T…kÎÖ?†1" Ü.?(Ów¦?€2ù@b	¤?dFŒGFɒ?Y5x&"(À?"MÒ´(ú=?}¯î¯õuh?î¿ÌqT2?£ŒÙÏ+Ü?€LpŒ?H©Ué€?Ÿào,bÓm?>ÈÉ¥(ƒ?îÕTñà?‹.ò±¸Ê?r¢ÒÙÓYÓ?p5ÏB? VVêÐA?5VTûy?ìæÐÂX]B?¡ò9:U³³?•Zzi?''t	Â@?³'ø×ƒÖ? Eœò]ŽAGN4FGL J1201.7+1429?í°š¿´`o@R7UqKœ·À:'£.mѕÀ<'ÌK@!'Mš¾@oªÛ
}2?Ó?ÅíhN?םÊD\P?ýS'i#°@×Ç7a–¿Öùœ#6»Ô¿Üéwލ¿àѦPaAc¿êC¡É¿ïÿüÚ±'Þ?ïÿá∠ÎAGNbllOM 198?ïDîñS®˜?˜dS`+í?qT°Úž‰¨?v›ÚWÍ
þ?"õ¤	ô›?•`åjtàI?ïeî¡¢–?"öL{mY?s"p$›¹Ü?'&Ê©Ö¸?ŒõÌQPj?Š…Á̔?ì߇—&?£3‡÷¿ˆ?¤zÆÎ8»?™1mH?®ÆMOì?œ¤·_Q<?°oÆ?q>à£íg?x™MÌðÒ?aڍL%¿Ð?ƒ…¬ð>?hglÍÀ?î§ÐáPß¹?¦kP0õ	e?}|€-ˆ¶Š?‰xLÞN+?¡Óaã.¤?£òc8£Nh?îKÏãÇT?¨Ö
Xá}?ˆÊ	Epnõ?'ÑŒÀ'Vß?¥už@1?¢ÏŠeuÚà?ëŸWTiD?¨²7ÌÕC?§akÀBzÏ?›ÎzèL±¿?·T€§_t?£sk˜»‰?îªü#bÁÒ?7)¡-?ˆ'Ÿy<?{Žv«]?žWõ>ÃО?ˆk÷é¾Ç'AGN4FGL J1202.4+4442¿ÔI"*>{@Qw#x«‰À;7˜ólÀ<´"!Š"C@§§·§þ@xd"?Á]m
¦‡¿µsd%Ä`?ô
®ñð@/!Û¬º¿ÚícV˜¿ê"›Oe™¿ßŶƒ	_O¿çCO¢Ý¿ã¹Ë¾.ú>¿ïÿÿ)@k*AGNbllB3 1159+450?ïÊ0J?ÙVNêiƒ?P–¹ÑV?N'e°Õ?v͹‹ñH)?Ú*à&¼o?ﲍ=ëó?€M' UãE?VƒÑSÐS?]ÝåU/3?€Œ6i$…?|dYeˆÛ/?ï,nÿ£J?ˆŒ¼fx/?r¬l¼¸æ?tÔñõ«\?•Çá¼'?†óÜè+?ï¨Õ<:¡o?epûl$È?kÀ_x'êù?X"킇SÑ?}µ2BšžÅ?_çV!0ž?ÛòÑç?•Þ#ÈmRÐ?d—¨
âF?b
Ïò×.?‡ö_ÉýÈ?"_üÞÆ?ï$<¼¸œX?™åk*û"&?h˱p…6&?wĶ"pS?˜^ò6KA?–¼E]Z¸®?îv¬Më	=?"÷–\Êǔ?	Șm=?{[,¬rm'?¤´mÄ
?'Qù´ñÀ ?îÊûuùù£?‰oñÞUœ?ˆzâüv?Wǃ?šcÇáúˆ?äŽ/d8èAGN4FGL J1202.5-0528?uÄyA4@K©›ý÷èÀ:+L''ÙÀ<;µ%ç@[§c0ÑÚ@OãÖԎ?Á¸v¾ù$š?Áâôq¯›?öcLŠÅÁ@ztJ»?ïÿýaw¿çßlâj¿ê˜"t¼j¿êzª@/ðÞ¿ïÿv}_Ò#?ïücÈý4tAGNfsrqPKS 1200-051?ﲎ)àí?¬F¦‡²Ÿ!?ÚHól|?¬INÝƊ¸?HG)E"Ö?Hý©WgMÔ?ïÑ)Es§˜?yUŸL¢©?LŠ—)¿?_u3óGkí?séÎYY?t&4ob×B?ï
n!Ø?"˜"2'Ô?wËxjÉN?€¸œEÈł?˜Ê"–ª7?'Q4Š}S?ïô%%ÿC?<õH§¥†ü?9ªj8îí?%¼$¬%'C?QKIvB\?7º5õܪf?ïëQ
šÉ×?s•ydsÇ?a¦™W.?sr{¯c.r?8F°%'¯Ç?=æm,UC?ïiÔ½\?˜ôbÁTïR?ZâüY~‹?qœÀ¤¥-M?'.¤Þ:@??–öžóĵ?îÐ_ótp.?"záË÷
?ƒ½…Vø|?‡CxÁ+Æ?œ>éeWõ?Ž[3À<i¿?ïÑaZÔ?bl"iÄ*?Z†?í§H?KK}¤ƒas?p­íhj£ë?]o6"Ø|AGN4FGL J1202.5+3852¿ê¢j÷ÖÌç@Rœ;÷'jÀ:h/"BAÄÀ<'{ZqÍ@d[ô@ÈÒDŽ?µg×)È¿¬×ä>Œ
?õD5¹ö0@¡$29c#?ïÿíáoq'¿â£Éh">¿êsҕc©ô¿àyÈþáòÏ¿ã=š)âQ™¿Áù CVíAGNbll3FGL J1203.2+3847NVSS J120257+385147?ï–,*Ý?ÖI$›ä?X­	¯nR?_WDyj'?‡_Tp¼øç?Œøé»cü{?ï¦ÛBþ¥?w}å'F?P~e°ú?TnD¥M6R?zC)=n?t´XNÛR?îÞ©rZ»?''?¢èY?o[¥X™¾?qªêX«? µQ*öì?'kø\Ù°ò?ï¢áí×o¤?c…`ÁO¯Ú?t;Ā,?ZPÄÌùÇ?zTpÄA›?Y	h†i¢™?ï-m¸"K?•d¥ ~?j^Ç¥·ZX?iîðar#?—oó½Xd?"ÅÇ
â?ï9û1£?•îÐ(±ß?f¾X¥9‰.?p4ª‡Øó?•èÑÝz;}?"] Wéiô?íñÛ¥ל?›	Áö?ö»2?€RüóbÂ?¬ Ǖ?˜×dõ/éé?–Ò6f?†ÚÀ
HS[?"aqèƒ?C?вîæn?—‹»9ÆX?|ûÅ:ËCAGN4FGL J1202.9+5141¿ÑvBwî¨@Oå¡ÊÀƒÀ;CZPÀ<¢¬k-u"@O€íl@'¶'!%?Á"íå÷K¿´í¤ˆµñ"?õÕÛiGÂ@]Öÿž?ïܲø¿êbÑñÏ»•¿ç¿:¨rzq¿á×¼_AY¿æ¶ÇÝyÃ:¿±?štµßuAGNbcuTXS 1200+519?ìw 6<Ž7?ÒvàiF(?U•'b¦-ž?{iª¢X?"?»ð©­°IV?ÒnðD»?ïIƒÍæŽ{?•Êj"?ßá?sHí§]ª?{Dº¿ŽÌ?'ýJÖÙd7?'tîñ81¸?ïBt¤l±Y?…2Ô,W?k"y3¿í?i±¸/@U?">Û:¬Vé?ƒþ"/&˜?ïmöX"õ#?qȯlû½?s©qÀB?^Í´¿<þÒ?Š­°ój×?l@´mHA?îæÍòð*¨?½››3o¥?a›Sw?SÄÐ×®à ? Ïã؂
?½¥ò²(u"?î'Ël®Â?£w­o?ÅÙÝdF<?'3Ô€à?£aÒ¼|§Ù?¿™<\?îˆvîÁ5·?' ýÈ	œö?xãRx}+?tÇÞP¡š?¤\&ÄÖWg?'Pæî×?í .¾ÚEÜ?"…À›Q"Ì?"èš#PhØ?"Žç΀¸?«ˆÆþûŸÓ?ÌgÉ©1AGN4FGL J1203.1+6031?µÈ¿ZRÅ@Kη#îÒÀ9zû¾QßÇÀ<o*þ±K@vò	óï@n—Oß;?¬èÿ¡?³`ËqØàV@^—eóS@	'R á·k?ï7Ÿçòm¿àBD]§ûÝ¿à'Y«m´¿á*i*f¿éV[¡'_¹¿Ð¥ÁۂOAGNbll3FGL J1203.1+6029SBS 1200+608?ïÏ<K¾M?‰ƒ*le.?[®5©£?j~Aþjè ?q¡ÛÞôQ?ƒœÚêc?ïE'îe´÷?—[‡'`ù?ygÞå??"¶mñ½J?'{Ryà?ž1߉?ﮖ/Ï?zàg0SA?dâ{Ð|,?rŠÖ$'Æ?~Cª­EÑy?rŽ§ìLS?ï"·=ՉÆ?wkÃm^šn?'³î73Q?q°M"û%®?…ȧOïê?dÛpréŠ}?ïuBôé˜Ø?Ïc;Ié?u'î6úG?rìäEœx?‡æKªÌ''?…Aõ:Ñ£?î-4ÝhŒ˜?ªç1 ü?ŒèV-Bµ?šIŠ(0¢j?¦	84Ü?¢'
õf=?ïi#՝*ô?†!ÈýŠYá?q¸êa'?xëeÜ®7P?ŒÚ•ŽýFX?€+i°ˆÌ?íÀð—µÙ?'µSÈú¼<?¦AÁˆ¤hz?‹VMªÝ؜?›^zP×ÿ?'³ 2iAGN4FGL J1203.3+1119?Ú5å%oas@Q¤_ !¸À:ç²7PþÀ<oIÊFá@7½%•ç@9'åøí½?͎8½`É?ÑޚTª|@iåvç¾@Ú¼ñ?ì[²BÝË"¿â¿ˆ¬Œ%¿çŽx¾­¥?¿×ž·æ‹º´¿ïÿù_|è3¿Áœª2AGNbcuTXS 1200+115?ï–JymKª?†–-X?r€^%EÓ?q‹/|z?-2YkƖ?KÄéÄ¡?ï"ç»a?‡@Al9—¯?iòC<2eÏ?nÊ?ˆ{µ5´öJ?'>V…{]?ïF\倚?‡»^—8a?zƒ«®U…?|[¯æN‰i?œ	 ±\?'É­áä±Ò?ïºmh}?w¬x3‰ï?‡««/'@"?kmÇöҙe?"ÜÀN¨ô?r‹:Î`ŠT?îÁë7ς½?¡^U³qÏ?ˆ©w¯n?Šïëð/{¹?›n
Èт¤?™@gã¹ÚI?¿ØȄ? REíÖû?}É
 42ú?ƒ3O×éip? ÜÂ`¨°e?›Q-U^è?î– ÜՔ®?"B¡'t£'?…¯eÔ]I?"ö‡Ä£5?¡-FXU¶Ô?0…
Xs®?ì¸Ób,á?—ÞQ¡¶³+?£Ñ"2wL?~¾ë6?°Pã&PWÎ?'tBO¹Y[AGN4FGL J1203.4-3925¿çÒS"/@6'‹â÷±}À:?Ï)è1À<INiŸ
@!*øé‹I?üב#'?·IӞ"?p?yùø²ŒbW?Åù çÁÆ@BÝJHy?éj‹#µî?䯂~õÔX¿ÞÀù"æ¯!¿á£œ*Øò¿ÒÜÍ Öy¿Ðå×?—ožAGNbll3FGL J1203.5-3925PMN J1203-3926?יִ´Ó©,?pŠÀýö?VÐcö˜¤Ü?Ex´+õ–?þ†O²<J?n|LئïË?ï¯Áp#Ù?ƒï–çêµÃ?S×ý伝?[]É¿¾$Ë?"¤5(©¶?'fß×ÇIÒ?ïX2–«'¶?"þßy9?cPÀñð?[@ˆ!?'‡£*šî?~BÿéG²?îˆø^mk
?'^}~MëH?{`jqb??`¥ª¤Ñ׉?¤w,3?qþUtt?ï)€rè;#?Šoeñò?o}Rˆ-v‰?``ºF4²,?–àGO‹2Ã?ˆ ëFíø?ï7ÉðEð?•—¼ûC?c&V[n,?qåôZj7·?–¡÷#GÑ?"¯t׀JŒ?îž^8UÃ?ŒÁïÙT50?qüÎØJÆV?p ¥Úù?£Ú'£ œ?‹TSQQO€?ì{µqÖ ?š¥ZnÀºá?dÆ~)%¾?|€Lí‹f?ºúð²ÁD?™ôrÀ" AGN4FGL J1204.0+1146?åUÔÖ0£·@QÂûÒsÕ»À:w<
rIÉÀ<a
ž¿s@ ž^/‹2ù?üƒŠ´#ˆ›?ÄE´£ú?ÀRb"‰î?þy*X™J@
¢î$î¿ïÿýaw?ïÿþBe«+¿á1õ°ñ¤ó¿Ö¸_˜1¿Ù×i]ç'Ê¿ê0S'ˆAGNbll3FGL J1204.0+11441RXS J120413.0+114549?8–
b?‰=æÖ¾\)?PŒ	 '²?DûÑ?qø?ŠX]x.?ˆâÛL¯j˜?ïÍ{ûÆVÞ?w¹©ŸoH?PI›á™~œ?X»u³÷™?u/›2OÐN?sǧzr?ï1ÏRZ7?Ž_ |÷G?g1H	̍?qý;Ü¥_?–䯆Yº ?ŒÓOŽVÇ?îåƒlÜw:?uw'Ãt¦ö?"
ÜyJ"?fg‰|mT?™CwÀF{?rHÚZÄ
?ïmWwÇH?MП="?f'á¾Õ?`òBٕœX?ÞNE'?däÚUc™?ïeç×Po•?'¾Gþ$?d½¬I"Ìq?oO&O}G?«OåYÄ?ŽIMη?îlðÌò¯?–"1Rˆc?sk«©¢_k?x*fr³ ]?¦Ã‰	Ý+?•_Âàÿ?íhµ.ëë?ý"i#È?•HKTYvþ?3*ü
X›?®Ð'žÙ?Ž3C×μAGN4FGL J1204.2-0709?ïÝÌ2n†@Jî`RP/À9nsbÎ+À;ÿ;"G@çß†Î?ü«åÌx7?µ#	ðCÊZ?µ—ÈAíá@.º'®›@—`,'?ïú·‹òçê¿äa©0'¿ßÝB»¼Y¿ÑÀ· jÄ¿âå4!Å¢Œ¿Þ•P^½$¹AGNbll3FGL J1204.3-07081RXS J120417.0-070959?ï÷ñ1õµ=??Tåò?#¹éìbó?ãÆ͝……?KL½4Ïs?;U-ã½>}?ïÐÜalô?t/DR"?N•Î\KAn?WV+µÚO¿?s¿¿ô®?o">mòà?ï«)ôg'Ù?r'¿8š:P?ZvÜ;QP?N$>Ò¬?æÂr# ?qG©9X<?ï3£'ä5?pûzÁí\?vìú"ö?WdzTb3x?"ÐO‡eÌ?mš–f2¶?ïõ?CW?GÝO'Ègz?0j=*8?$¶‰ºzêb?Q®Þ"¶c#?Dà#©%?ïbò~Jf?WJú4ú?c
Ä°ù2?kŽ¥YGBT?'?÷¡=¦?‰Ö8Ä2BŸ?ïu'<3?d‰åmÜ?cäːÉ{³?dèr¶|"?¼þÊTK?å~n¢Ïh?î	™Œé;?‰¸@úe?ŠkŠ¢×D?q™ƒ¡™?¨ËŒr€?‡.äb¡ÂAGN4FGL J1204.8+0407?Èú;J@P7!Õ<ÞÀ;?ÐÐgŒÀ<~ÐV©Z@xB÷¡aº@ØÄ$"õ?Ðú? Ò2'?»æ;èך?èýpÇZ@	}=*WíR?惠žp˜ï¿êÉüÙ´¿â~wiÃèø¿ç5Š€Ìï¿ïöþdŠ¿ïÿñQçSaAGNfsrq3FGL J1205.4+0412MG1 J120448+0408?ïâ!܄áã?nА9Gl?Eˆ"º{^?BÁnÿ'ÌÚ?h|¦·£ì?jíe/YÆ?ïÅéEuÍY?vUx)Þý?N×_ˆ,?Tå÷ľ?y0zž8.*?s¸Ó¦[?ï|EmÈZw?'ËúbYØä?a™	é??dñ÷´A¨?ŒˆbL–Õœ?¦'Äùò²?ï°È;\fL?`Dª¦Ê–$?cD6€7¥`?H~`ÿ×}?}ùÆð´Çi?Z«nÜ\?ï®/÷4G?'9v÷^Ã?SûÄW˜xH?O(F–8ëº?ô‰¼Æ15?…øTËk?ïH.Î
ƒ?–'KzPè?aó<V4?p<*Ȕ{?"±²Ÿaö
?"Sýö=óü?îíØ¿¹Ù?DRmÊ®›?köñr£R?pLÀ ƒ?žÆ	ãN['?hCÊÕݵ?ï")"ªÊÍ?<"ù©Q+?u§Å;;õä?d´"PhP?–PÜ8í?|rÅ3?6AGN4FGL J1205.7-2635?ÇmW"²@A"÷ µíÀ9mc¨FÇÀ<$
­,*@@SÃ÷f(@¥­Ûp?¯—d53¾?£9F? ô?ñ*MFðP@
cÒÃù"?ãR+Sk¿äå^ÿiؿ跍¹ç¿äNüm¾I¿èñžBuÆ¿â¸Æ báwAGNfsrq3FGL J1205.8-2636PKS 1203-26?ïð²qÏ«?M²êwåöÃ?=Ú8ƒºï?,ÄOtӜ"?W$Ž
¢—?JÙ áà?ïÖË9Š÷Q?rÃjv?I@¶»´?U$"ʸs?qrL"‡Ø?mOŠ3π%?ï¹a*ðÍ?q¡' FšŽ?[žëÖí?`RH?"w™?|ŽBÔã?mùÆñ1?ïÏq…‰ö?Uq6ˆÜÎ?cÞ"zËBŸ?Gã=²¤?l°½Ó¯ÇÞ?L6֑SÈR?ïÛÜøDž?e­0"[h?P©<Um1?FεÉî*?kÎhÕjÎÖ?bÃnãæ)w?ÀM@-?ˆ"S}'A ?`¸;òÃÛ?mÍl ¸?ˆ¢H"yÅ?ƒÓÔós¿ê?ï'Ä":?}«‰?^+±?gÛ·kO¥ù?i¿IÑå e?‰WñÞ~x?xÖm8S_Ï?ït*ÄϨI?vAì6Z<?Üo¯Ö/?jI= ÷?ƒçy~£?i""/"ãAGN4FGL J1205.8+3321¿Õ¾7©öš7@S—àÞ҉À:êj€§ZLÀ<'Æp'9S@réîñÐ@
þ`Ï6?Åhî
¿†ý±Wa¡í?À"‰õŒ´"@òý
':¿Ö® ¤»5Ì¿é9ˆ·Ê¿å½Ëb>Ž†¿ãe"bøô¿î	܍40‰¿ï½ A"ôAGNbcu3FGL J1205.9+3315SDSS J120542.82+332146.9?ïÜ¥/Øhj?i¼
êâ³?MádŒ=Âh?B ïÍ3A?kâvÂ&)?g^œšäH?ïÓ¸Ãøµ*?xdüØÒðJ?HLý®¹Ç?S4*Sw?s¬HÚ?uÿø£¶B8?ï"ñÿŒ<º?~̕ÕÝ?ZOžÿG¾?]Nã1Mû?‡yŸÜ²P¨?~ú,¶Ã?ïϬ™·²Å?VZù0½?^Tζ{7?E	Ø×waã?p"¯&**†?R©§(Wrè?ïŒf~Þ?ˆ'W
g‡Û?aL™—|ã?U®yj(?ˆ"Y ž)M?‡OÛ;xǪ?ï…:Ÿì¢‰?›`´™ÑØ?S>A:§*°?aÔÌ8X.?ŒIæÉjp?Œ%Ÿp*«?ï E¦q?‹ûóÓbB^?bD9¤"/?\Ãɋ†?™®Ä‹¼?‹IB!	Pf?ïiõù'.ÿ?vº["Óò"?wþHÛ¿™?g!ýÀ-'?‰ƒ]Q›§\?qSÞÿTøAGN4FGL J1207.2-0524?í¨sÃ@Kàw¯dÀ;ÜÂä¿À<œ¤ÁëÈ;@ ™o¬5R?ù-Æèk?֒ÐÝR«ô?Ý
³ö«˜@x÷…@±ü/æÍ¿ìNá¿Î¼?ï{ìàh‹¿Ñöã•Ò¿Ó>úç'Jñ¿ß='üft¿ðAGNbcu1RXS J120722.5-052442?ïÜƊ=†?d[W9ÛÃ?WŠî°HD?P[­ˆÀ1~?hô2¤ex?^œ¨HU?ï½æ] !Ò?z­œ+ø%?Xµ­–¼'?aÜ[ôê'?zßeÈ0+Ô?séÚm¬þ<?ïL%Û0è«?…ƒÂC'7;?yÂÞÀ?~:•`l*?
%v?}–7H›l.?îÅÜ軃?zÏÎ'¡u?ƒ—6'…B?hµð]dÐà?xâãç$û?uÔñÿú09?ï¿UFó]?rºBpÍz?hyçÉ®Ñ?d^¿Tä?thªÙõå?gm*ÃR›?ï?ïَŸ?"r©J³z?j·ú—éÊ?s¯ÜJ"?"Ç \ä)?'n?êîã?îÃß9¥¬ç?'ØÚ×dpç?|P( '¿?é#ò,ì? 8
â ãT?>;˜ë?ípRˆ"/?"ˆVÅq?Œ<G6¨ç?:ó¯Õ?°õâ×¼o&?';C [Ø'AGN4FGL J1207.7-0106¿ÚÐnˆÚë°@Mï÷øʂÀ:"ºˆýj$À<e*F$§@Î]Àz"@ÇúBPÝh?Àø==ù
?ÆÚ9ÝFl¡@ŒXž&Ç@éÉl|«?ïïZ@hOö¿ÑiدY¿ç&Zݜ'é¿á"?B
;˜¿é>ê¡tˆ¿ðAGNfsrqAT20G J120741-010630?ïÓk<íyÉ?–beà5‰?i¥5	TË?–v¸Pæ?bïÒs"_?SŒ\IÍî|?ïÝôö¡?m~øÄ[<?A:¶¬yí?I÷1Y×g?m½OÕÍöÇ?i:ÿb§¼0?oN}£?|£5jA"?pGãÙU´¤?sÛ4[^Æ?ƒnrP‹Òì?t€5Sû©?ïèä:Û%ß?Dé
Ó7?Kù?êFÙ?0ˆ‹pQÐ?`u[Ãr?Au¤?ŠÁ?ïÄå»í<À?r4€/NB÷?kÏáæJ³i?h‰ßɤû?oJbbtB?c³v<j½?ï">èaíu?‡>]'?T?HX¢?`"(ìLâ¹?ˆhe¾!˜"?…k¾-ç]·?ï%Ãõ¸©?‹dH59?ƒ`Û=ýi?ƒÉIý¨v|?'›ÙÛk/«?€'Z·Ô<?ï½bmw@˜?dŠix}j?dZ:–!g ?Oò»ÄJ?w!«çqA?`¸°šWQAGN4FGL J1207.7-2229?åH&IaÉ@C£vfœíÀ:[§ºÄŒŒÀ<e¬9¯@DÛ½€?ÿ¾›ÌyÀ¶?Á7°év?±ô¬¶¬Ð?ñãUŠv(@Š`Á‹Ñ?ïÇ~¿M³<¿âg1g™¿ãåóö¿Ûp°½"Û¿ÞÆwž5@¿æèþ[»AGNbll3FGL J1207.6-2232NVSS J120736-223036?ï哒:÷ð?T$Nó¾ã?ANƒëýÖ?.!¢ý2ñ?fÌ­ª·?Qët¾Ôø§?ï܉ûÝN?n¸¦Ë>€ç?A™‡Jæ?J|1Eƒ7¬?o.U¾i?j‹ñ"h@ž?ï¹
¬¿?l•Z+Wå?Rd$É4P7?9 싀L?~à 'Ô Ÿ?k{'épuJ?ï"/nFsq?`næ¢ÁÍt?c5aÅ:Z??ŒY‹}ÊK?†&áb¨c-?^óc C?ïÎü2Ò …?cT¿uMk?Q =US¢??‰·CÜÅ?t×FjHü?a:ƒy¾¨2?#—ù?†@¥ê~Ç?T÷<å÷Å?]§¶6Û?‰tÏy"/f?"8¦ƒòœJ?ï"r±ÎD?x‡b?ÔA?\ŽkědC?Iô?Ì.g?‹f•ÌŠ¦š?w¦;C?îޝH?}'8|HP?y`é…ÝR–?]DÛQIô–?ŸÑñøöä]?|QmãθAGN4FGL J1208.1+3017¿î9ᇆ@Sÿf¥P‡À;x+¾Ê«ŠÀ<Пe‹u@!KQŽ½ók?øœ bv?Ô\™`?ПäâBTä?ùÕ¢y<,@\<ŽÑ"ˆ¿ëÀnºÈ¾J¿ïûmÊö?ÒÊM8ßð¿Òk.óŠ§¿áì^Á¿Ô1»¬éØAGNbllGB6 J1208+3015?ïÌRëy$?l6³©¬?Näߢ™E×?E_—kÂk?uùîI›hÊ?j\âD¦?ï–ÕDž@?‰"3K;P?\ð6*?f'{ঔn?†ÇÒê€ä?†‡)8Ñ?ï!»‡ç%Ð?‹ :J89V?eõä=ï´4?eWN̐ï«?™	Òv5å‹?Šb7̂̏?îÓϘâ˜?{©Îm¨Nd?cÂùÝüé?NÈ.1ûðÖ?¡†ÖÒÂח?zúl¾R_@?ïŽ/íû½ó?€vV½¨?Z&ŠáƒC?OÍ`g'ŒM?‰/3(´Dº?
Šl̦?îÊ{%‡›b?¦âóëÇk?og9$WÛÜ?{(5ôÆ j?¡aÚöñ¨?¥c2`l«?îCû¸¦,Ù?–6ȇü_Î?j‰‹Z?ÕA?dÙÆï‹é+?ª«¿Í:$?–>í`¹?ì›-Ãæ&ï?š¶5ßõn?p=1¬ÿá¥?bZ• -à?º"¾Æϲ°?š%Āe$¤AGN4FGL J1208.2-7810?âÃ8DÑ&ŠÀ/d"À:¬#Ï!kÀ<hýwƒ–@ =÷¼d ?ÿjj6Õ#?ʳiäËG?³Ÿ€ŽZÌ)?éõv¤¢X?óŠy?­¿å2 -"¿çâ/jPÖ²¿Û¯~ˆF5¿Ûo/BÄ#¿á@¤Ö
¾/¿å!	ۂrAGNbcu3FGL J1208.2-7810cPKS 1205-778?ï²D˜Ð
?vT¬Ÿñ¦?BÝx¤B?9ëùçeì?'WMMt¿?u¢UC&?ï|ȟZg™?Œ‹BF?f¢æNœÿ?j¡'mr¢ž?‹)¯qŠ@g?‰mÿÓ©C?ïcÂϕKy?}›mþ7f?f¹A/ð:•?gµçŽ];?°}ãdüŸ?z¥Xíì|÷?í,¿e¨rÈ?Š'Ô±Ý-#?†3Ÿó-'=?fíù9´¤?³ÓÒžé}?‰ÙÑjÝ?ï`€øM?'Ä$ñ…K?Rq‹/ãæK?JG´"?'ÈÕ¤ë9þ?'Fò*ö#?øÇ7É?¤/ëÁ?{ù¦$|ð?"(6¤³w?£Å«­XÃZ?¢nþêï?ìÔ»??Ö˜?0Õ?r!Îʑ}Ó?p68ë×)?¡áG]U©Q?Íóó•)?é	0smép?£"–y˜a$?–Z6–åÁ?ƒªì0¡ÿ¶?Ér齯Š?£Î•ÔÜô_AGN4FGL J1208.4+6121?ï÷whä'@K'BZîc À;Gy;UAÀ<ãÚ\ØH@þèL/-•@ü÷¢cl·?Á±Ýˆ0æ}¿£ýÛb'Ő?á¨áJÞ @	·ïEÀ¿íÜ3rSοÚ\uâ/_"¿æoÚ•[œ¿â,ûv-ƒÇ¿¨`Ž­K ¿ë

"ZAGNbllRGB J1208+613?ïô­x7û?Rl>],Æ?2t­˜&ln?0¡Öw?RãÊ¥`8?Nùò`Eþ·?ïâÁñ|"‹?mµ
s%Þ?6À×ùÚLä?AX!}¨§ÿ?jeóz7µî?kpq‹WB?ï€f¼ÄäC?"›åâ
ù?U:©3"{Ó?cH"ÈEÃH?>û­#ÓÞ?ƒÝ+Ãhý?ïðœÈx)\?Dx²I±¦?.,wnó(t?–\¾Wd"?[àÝ~õ?DFËSøt?ïæ‰ñt¼?l并ý#?I÷]47l?VE²óü÷?cº8C¿ý™?eBð¤>p?wäW?‰,̓vQÜ?Jòs9…u1?U'ëöoö?ˆo±sê?ˆ*¾—¬?ïR$¡0M?!¼cÃà?aJRç¿?n£0¥Ÿ?šŒq¡]§?5G,ä¾?ïʘ׿Ê?fz£B~"?IÌy"»>?@aéĸ›G?wÚîÃÙ?f'Ô¼ü'^AGN4FGL J1208.8-1751?ïNŠv³]@EêÖ¡aä÷À:ë‡ß\òIÀ<~ϙ/çN@x¤ÉM'X?úøihyf?ئးø?ߚOa'C@I	¼AdN@JdJ,sü?ëÈì}—/‡¿ìWàðñ¿ÑƒÞÐZv¿ÜgŸKŠB¿î]UE¬²¿ïÿ韖]ÐAGNbcuNVSS J120856-175647?îÑ¿\¼!?›`¶ÐÁ?…`°å'T?~žÖçMAª?›ÅMåV«?–ÁÊe>s-?î}‹…üü?ž·þð?'×˱ÙQL?»^·ÜªÚ?žvÅð'A?Ë‡ÌiYô?íJî"=Î?Ÿ±"ab²?œy¹0a€?'°\ä
"n?­!dCh^?˜Oé7ˆˆ?ëËр¡â$?–'"¡Ãô1?¢)›-84‰?‡ó°8æ}?¸Œ¦f¢›?'ãÜ äÃb?ìÜãßýšå?°? Ó|lÍ?¡Ù>ál`?šºqÌ
C¼?°,A\øÖ?ª¤.‰Z{?ëÒI	Íøá?´i.g:"ˆ?§N"mÍÈQ?ª,(v9/?µÆm{ó/Q?©õºkqC?ë>N'š+?¨m¼Ë;Áç?£Ú@(¿/ä?•þó¥#œ…?¼ o²ÑŠ2?¤¡òO‰?çÒNTÝä?©þ–q½?¦téÿ4?›Ƭiƒf?ËŒCÛ?¦ø²bþAGN4FGL J1208.8-2754¿êšÿoXÊ¿@AԀuÀ:œ(MüãÀ<añvÐ@ö@ˆÂ‡y†?ü~†ƒ<`?ÔS—VÉ:q?Ó#ç{NÕÑ@Ù櫛#Ý@é?'³"W¿ïÿŸ½ 	?ïî'ð2,£¿ã°E!óé¿Â½§€b¿èÎÁŒ&ê¿ïÿüoQÇsAGNbcuNVSS J120900-275350?ï@Šïÿú?#^åú¬j?y
]5—ð?sº‹QI?'»÷Râo?‰ZcˆA€Ê?ï¶"ÀŽî?€¨¶¯_l¸?`ŠÀÿ
?iݞê¾{?|©ñ3³³?vç<sÓ~C?î»äš…Ó?"ÍÐÂu'ð?†Jk,J–?‡BfŒ8ùj?^G4Ò,¤?ÓÞ뱊?îDÚ5+¨?ðFå?à´s*=B?p1H—~>?¤:2Ïâ¶+?}ѹs¼)?îSáŠã¸? ·ÛG"?(>á²Ð?‰KSšÄ­h?¢÷חŸý?˜Nú¢¤Ù?ï#GÜðí?•^ã2½—?vfÝÁÔ·?‹fTN?•ýdԜÎ"?;Á]i"ê?í%®  o³?£Wd®¿ìK?•bã€Ê>?'ŒÊ§yCG?±z	Bø6Ù?ž¾Î…ª;?ì†ÔçÖò?—°·îCj
?–Èæ/Á±?‡(œ
Êú´?¶GͬÃ-?"-gn¤æAGN4FGL J1208.9+5441¿è'€4»@N­gý?[`À8¼iuå_kÀ<Bá³
Þæ@Œì‡¨*@é»ðÜw?¡$åhd1?²·z«ð@`"~@'¤¦½ïd¿Õï5­`÷¿äþ'"o¿çñ¢4rοæñùý‡¼¿î™pI>7s¿ïń~ªTþAGNfsrq3FGL J1208.7+5442TXS 1206+549?ïäàry¢·?'‹Æ¶Ÿò?PÇ+Žu?I-Ó°Ù¥?b»÷ýO?'{9ÕäK?ï¡Õ¥Žoo?ŠtDفÖ?aæ•[«|7?v[7ð?ƒñ>š
>?…\H
:?î÷œ.ÒÙà?›ŒÏ¬‡$O?s×óÌ1ó ?{…Ð
XA_?œ}:«\?š†ðÓö?ï÷­	§¸Z?6áÎHóó?CƄËioÂ?1RAC&ÓL?;
ªv^G³?%óúL?5ì?ïÝ?²Ú?h†ŸÒ¯Ä?Uu9ä
®?O,CÈ´;À?hZŒn?d©‰0Ã?ïÔú\—?¢¡)&‡+Â?p¢—ÕÙ?¿?…s'||˜Ñ?˜v_oá–1? K(µÞ?î2Y!7?¦â"ýäz?{`Ä ?€ªe`S?ªð׫
?¥®rzÐ?ïéåƒ@Öy?XK'¼I¬M?[§¦îÝëó?R‹zê¦UU?PRÆnâR?C‰Ð'"PÚAGN4FGL J1209.0-4630?ïìS@ÕïG@/~ÀÖõD»À;"G¡A)À<`émƒÐ@0\"*š@mgâghÅ?ÍçΰқC?£ÝT Á?ٟ"ÛCÝû?þ›©¡¤ý?è,ck	cV?ÍYþí[c¿ë7»ûS¿Ðzý©8ž¿â£Ÿ¬Ù¿ïá½?6.AGNbcuSUMSS J120905-462944?ïmß/a'É?†V$Ôê‹K?S9ñâ\¶L?I
ªKŸð»?'zúÜ¥i?…¡í*YR©?ï@žmé½s?­4Î`B,?eÂG]˜©³?m'pr*Ø,?•3éN~6h?›ì5^5ßC?îý€¹â?ŠÅU£å<?t®ÙQ'€q?sþdGå^?›$F[Y?‡Eh€L4š?ïn×½Û\?wwÄã{ÿ?u~ôí?ZæàÕÞeq?—žÒ@?tÒkólV?îÚ¼V²ê#?™€åqÑ?c§Ð~*C?]-rÑo#?¡½Ž'ë°?˜Ñkì,ür?î2t•dfî?¯ÄCÊÕî?zú\C¢ ?ŠIéÌð…¥?©yk%àÖ?¬mmálÝr?îºW̒?˜fGæ&B½?'nY•k¹A?}xœMýZ?ª˜Ä	ô?–ບ?í—'"Í	¼?"
|Qv?‹'#à@-?ys,­"Á?¯¬â¦Ç¸7?Á"ˆÀAGN4FGL J1209.4+4118?ç'‹	^@RY•ÔèûÀ9¯¡BÛGÀ<N|c'í…@^owG?ý¥óå?ŠZ?´åp‡§~µ?«Û^¸r?öÖ»cý@]–ý]
¿àˆÊ>}¿ãš:Þù;¿à›T\ÈX¿ÐÜÍ`pƒ ¿áf¬ƒ§À¿ê†#À¤ukAGNbll3FGL J1209.4+4119B3 1206+416?ïÞ8eTÌ?i²hÉê.?CöïX³°Ÿ?3ê -x??lÉß݊?h;;í¨?ïË$òäʬ?w(4¶šÎ#?L¼z"'"æ?TÃ:û%…?vÕ÷Bí?t9{S·Ó?ï‰{‹DJ?xɧÿùý?aÑ@½õðc?bWû9}ÂQ?‰GåÊWy?v¬Ñ¿.›?ïp^@¹??j~ÊLˆ?u¢Òb˜èx?WžµÐ˜r?‰'BLÎ?dtÈÖ}b?ïÉiiêÄ?eŽ'ÙѸ?R±¿ûå?@¼?±…?vžÚùÌ?cRö3ƒÔ ?ï]cW2t?'èæ͐?]Õ°‹Ï‡·?fPãnjo?'v:i|?úÞÿ Ô?ïâç§Ç?‡3"`4ñ?oVÙ¡3¦R?p\^»¥E?™ØÇÐæAP?…Yœ#mµ"?î´»]†q?ƒÚ=š]˜p?ˆªÁ~âû?qúý÷7©?3‰Ph|?€JPö…ŠpAGN4FGL J1209.4+7608?êð¿P•ø-@D\Fà!qÀ:¼¼Š_ióÀ<Ön%wˆÎ@ÿ˜Î˜~ç?üñÊ,ß\?ʃ2yúÂÔ?Ói¢À^Õ@YíÚcŽE@	PålU闿ìëF…¿ºõ¡Aٔ0¿Û·yT¼¿Ü_G£­™¬¿êñ0š¿ïÿJ-J»æAGNbcu3FGL J1209.9+76072MASS J12093020+7609120?ïÅ[+Pœ?w« ŒµÙ?eç`'Ü2³?a|}É?r^º{¶Œž?qdð}oö?ïÄ¡8'¹?xÝ:~d2§?Y‰Y
(g?aÆ*«¬?wm%ÅQ?r$1öbÁm?îéä@LÝ?'2¤¢I1?Š]6·®å?ˆ#·©ÊË2?•˜ð$¶ZÕ?Š}óBNÑl?ï ÎÒ¿Æ?aØßíøS×?s³bƒ…î…?R蜄+-‹?{å4xª?XüWDæ?ïmƒÑ8ö?‹|"êÍÀ?}'Þ??á?uÿ\ÞԔ?…ÅïïÙŘ?"ùô$	ª?ïS£ ‰•ô?•ú¢{ž§?hóh.ý(?u.æNQgi?'m.àåè?'*͹$Ý?îF§¨ƒ ?˜"Bˆ?"¿œzÝ\?±!CÁ?¡À_9ÎP?Ê{̚›ú?ï/ƒU+øÏ?|tn—°[ã?':VÀdŠG?k vš•?òiö[?u2âã°AGN4FGL J1209.7+2548?Õ½¯"hé_@T%sBí»ZÀ;|iÃ8èÀ<Õªøg…@1<¼ô½'@9±Y©¿'?ÑŽŸÀz.?»G‹.ò±¹?çÀÞöÅð@Ͼj´SÚ¿ïé‡þ'•ê?ïÏ[½•ø$¿Ç÷D…(0¿Ù·ª%ØØ¿ä?"=ßßy¿ïñ/DÀ#AGNfsrqB2 1207+26?ïÙ"òn?jm?³ÉŒ?@|wžž?0ç¤W¾?qgᰝã?iÆaÞ`£?ïÓu[Tm?uµ€!Î?HUoß1Y²?RWÍÅèÑi?s:¤`ú‡?r­ïñ àg?ï?D%"œ?ŒX;½ª?bàrÒ6l?b·h¹‰Bn?•»z-ÝL¼?‹¬›‡
.?ï}€Ï¦Ïk?ia†iNk?uˆ]䏺?YzVwß-?…۝ ìòx?c¿ìvVºŸ?ï½,%¢ÑÒ?rÑÞ¬^õ?M4ü\º¿Ê?@Lêjʪ°?}ÃM¢–1¡?qç˜àI÷?ïq	¸¡®?'â$?Yäl%)?al¼l.ˆÉ??{Š?'O
¨p93?î±7HIM"?•º=á´{Í?kþçÂ=?j+´VÍ?£,œþïWé?•=TIXc™?îÞÚ!ãÄO?"WÔËDqª?'×hðÎþ?rœ/É5Üb?š¹‹2™?€ñ¯ËVJzAGN4FGL J1209.8+1810¿é¿T¾•žÛ@S9,{‰
ZÀ9•8¬øÀ<IwëÉè@&ãÏGÑP@'ìB³Ù·?°–1Só?™6&`D–æ?å—4àh@i$ ô+á¿Í{.I"s•¿æD}ˆkõ¿å¹î£·*¿æe̽ÞGt¿èvuþ	ῼß0Q¬pAGNfsrq3FGL J1209.8+1810MG1 J120953+1809?ïôùٗ­Ô?G%Ʀ89?+RT Z?uIhpg½?R¢oV/#?E×î#s|?ïߗïí°"?pŽÒ/Ö??´Ö=לè?K2äØWj?lqu]¯–?lè¼_åS?ï²à@g?vŠŒŸ®Ü?X¢ÿyÀ[à?_pfpՆ¬?€cçó§&ª?t~!Qâ{?ï÷cÍõ†?2»Õ¶î_D?1&ußyþl?pV>òbþ?IÞMì7w?0`n{òãb?ïê¡#{°%?Y¨>`U…º?9ÝÍ$d,?/æû՚à]?b> ?WĦ¹4?	dWÃ?Šç"'1þ=?H·ì‰õÙ
?V%¡¨Co?†Ë>Ô½a>?Š/úæÁ?ïk&µTÚ?…æ¾ÝÃ6˜?eJ'}›Ó°?iŸ=Zos?ã²
Œr€?ƒ¹d#6Ú?ïæO‡?UÖëš|r^?JÒ,q·9˜?9dœða?cGc´_ä†?RLžFƒbAGN4FGL J1211.0-3800?ÝÔ·Ý|rl@8,aՈÀ:`~XËs0À<b$Óš@ð[Œm·@¶ûú·Á£?Â1²)³W±?Á2Ã6K¨?ÿ"Sd+"Ã@ð™§0†?ä±+¡nz1¿Ò·6B\Eü¿å;ÔÂd"¿ÞC5ߵݝ¿êðj`Æê5¿ïó‡K¹;öAGNbcuPMN J1211-3754?7$X?Û%e"?ù¾h/B?³]!æX°?šs°®©¹?¸¼TáW$?ïÊW±4?w4vØ~?U2(–TM?^	œ4$ÿ?u²JaðWc?q˜À^?ïŠ4z
À»?…'0ÙWBß?f­eSÃØÒ?lÇãZ.U?‡Çˆ"zõ?ƒ¨äÅÑؾ?ïY·R"rØ?fho•?}½'¶Mêz?V'¬néR?Š³—ŽÕÚã?bEî
ô'5?íü&W5NŸ?¼^:Œ²š5?›F™¯x"õ?·|¥ÙÔ?¢šM´îӖ?¨3\½‰ý‰?ï^M	Àj‹?'[©-?h'Ý'œç?q­è ÝĎ?'$|u?ŒñßâÆa¸?ïLoŸ å?Šë0úÍì?nÉ!'µ),?rJÓ=uE˜?'˜çåNpH?ˆt羦Õ?î?Sí4m½?ÀHZå?"Ô5)%â?rõ¢%{±ô?¢ ¦iÜ??}–¯êsè¹AGN4FGL J1211.6-2735¿ïõ%W8²4@A: _ñØÀ:?d?D¹mÀ<‹h~n›@@ï3@WM>w4?Áï$»v8A?²j(gÓ"ý?ïˆØ¡lKÙ@
©;×òp?¬˜¾A2"¿éµ\8;¿æçKžd¶¿æ—4d‹šÓ¿êoÔ;V¿ïþ§¥Ë×AGNbcuNVSS J121135-273615?ï°"7†¡?ÜóÎ}ØÇ?YÉ#——?^ºOBš›®?€¾Màâô!?Íœñ]"?ïËIí¬8?tQ"'h+D?Nûô•§_?U‡øž&?v¹{›[­|?q
ô¯"?ïlÙû'?"&óþ¢¯X?c}
m?oÞ»vC?™üÂÃ:{?"¦×n/ÿ?ïrbñ;ìë?gŸ9ö¶(?gM' PÇâ?G¡Ãýò?"ßÊiU?eé—Ä÷³?ïQ}"3ï?—ztÆ?h-®Ð§<?b–àכ²Î?'ʝ€U'1?–Jßùډê?ïj"¨	x?Ï}äÙÊ?aR…ö/
?k/œ^õ¡?‹à¨´°?‰J¦'­ª.?îKmφ?œÀ²2"Ú#?j(Çc@?nøza-_?¥ˆÈöZc?œ
'¾ֆ?îIƒS~y¥?‰iZ=Œs.?'nʹþ82?hò‡´!TÃ?¦ÌÙ'§?‡8ùÝj—AGN4FGL J1211.6+3901¿Äù,B9q¢@Rß`þG™À;Yá'nÀ<ÞÖÜGª@î',èÁJ@ƒœØ{?ŔS»d¿ª?ڜªVf?ä UàÝ%
@-=ÐÆ?ïÎá£0ò¿ëbS².»Õ¿ä+z!"4-¿Ùô¼ .ß¿Õ'äKn"\¿Ýõ3ô#RëAGNbllFIRST J121134.2+390053?ï£QoD—›?{ïj,ØÉÛ?I'ÌåŸ8§?9pp» bÊ?…™'o4à?{)Æ¿g?ïÂ-M&_¡?z>aÎçw?I¸•0@ï?Qи"Q¥h?{²GIšo¯?wÐÑG'‡?ïX"æÀO?'5È`ác?X²õùÕc0?D¨¬Ù7[ù?"pàòYå?'U^«ƒ?ïÈW
\?^ŽÁAZì?PÀ+þ…\n?7}ñ5¢zD?w¤oÔUڋ?]Š]~ò·‹?ï֐V5'?":	Iú?Y©%Õn?NnqôvKl?žJ›œ¸ŽÑ?"ÖåzNÂß?ïoÑB}Ý?Èåkçö?RWw"Ù®?\ë²â\(d?àhe8 Õ?Ž°¹Í"ét?î':[+Ûâ?"c¤t{î\?bJ'n0ðó?Z‹G—|\•?¥·±3s‡Ó?"4æc77?ï(¨©"?€¡h'?m"z8q¡?]k*5ª§?—8{
Eî?€kWæ­²AGN4FGL J1212.0-2326¿åÔ~.?j@CDQ£"îÀ:_bnŠ!WÀ<N>Ȓ«i@ ²WlÎ_t?ü‰ý_;Ϻ?Ĉ°'Ð~ˆ?»ã8)‹À?ùÎފdrp@	³l`%…?â}E`1n¿Ýy]¹ïz¿âLuĨ;¿ÐàØóK½¿áƒè¢–Bw¿ÛX£Ó¯AGNbcuPMN J1212-2327?ïó=êœ@"?Gx^pÑÚ
?%l>(0nv?-Føaê?VÖ£DþÇ?Fke»?ïØFK4S?mú°Õ\R»?C€_òÙh5?L#ûTßk©?qlíì
¤?icÌ# ÁF?ïµÂzõzÒ?p™z>ÒO ?R˜
¸<µO?Q>=°î(?€<_Ü{læ?nGÅÕÏbN?ï0²ïùD?o7,ù–`?f9ÄÚSŠÏ?Děy¡õÏ?—"imt%+?oª45­‡?ïì¢!ŸÚH?Qõ|½›â?1"¸™Ó?·}îÛ1?a9Œ-=W|?Q›Ù/ž¹?ïcîfûb?‡{!Øn Ú?U³–*†^Ò?_+؉æŸ?‰ð'Ÿƒº?…'¯
¬ãd?ïp68B³ü?'
<Qd€™?\àš)À?^\t	9'?+/Zjíz?Q+(Þ?íœ/¤ð?Œ˽º'‡?|aÚüaü?d0Ô¨s/,?±Xv.à‡"?‹ÃÉAG¶AGN4FGL J1212.0+2242¿°Þ©–'\@T½D¦"À;1	G|À<Ã"̳¢@‹F©\°/?ÿw_²íþ?ÆòT†?Ï?³ˆÝðǺ?ëöŸ™Û@ÓêÎ?"¿ïÿE€Þ$?ïö?ŒÝÉt¿ãI=Š¥
¿ËÉKãÙ-ٿꇥïaL¿×+¢zé«*AGNbllRX J1211.9+2242?ףּÔ5vÚ?yq&B½Ê?_|tµ&šv?UL^¿-?€¯|icð
?uæ
–» ¯?ïÁ[XÚüT?€ÑÆÓÙB?V½›™‡§?céR…2å?y¢ìººæ?{"¬õ]æî?îñ5=é3z?'I67œï?s÷x¶Bò?ysöY$"Î?œÛ'ès'?'µ¹oSÉ!?ï3ʱ®R'?s<¢ìSMÎ?‡Ð»ÜøZ?lëú'•\á?‹=5鼉Ã?f~	'õ>r?ïl1)vN™?…<®ûä9?pøÛ«-\?ié ÷=°?ŒwGÙ4C'?'0¶ùË6`?ïKöCú¼Û?"¢ß0Ö?g@ý×æ!?qW§CÁÄÞ?"™ÌL	É?'sêƒM<?îm\nk?–ƒoVg$X?z‰õXÒj?yšµÜÆï?¥çmkvJ?•º~Ôaå¥?îҟŸ˜?jrfY8?šßÈoHvâ?…¦ü4—¬ò?¡"ñÏ>*Ù?"@˜Ž98»AGN4FGL J1212.2+2442?ï¸ØPÛÝ@T6éNã'âÀ:ç{³Õ…À<¶tðlå@?EbŠ¹­?þñ
‰U~¸?ÉL'jPUÙ?ËÙ@x–Ó@'åøí½?þkÌ´Îÿ,?ïŽBî's¿é='þ¡±¿ØëxßdÔì¿ì{Ô!Tä^?ÐZ"ŸY¢¿ïþ"ØrAGNbcuNVSS J121219+244130?íß6åLþê?¹Â҉5"'?ò­J;8–?Žø獵°D?­æ[vð¹?·oÁGÍ7ð?ï19M ê?¤<ë,"#ƒ?sb€Ó*?"¼ÓÇyJ?•@1Ð/ù?¡+(•Óïß?íÎ
+ÑY?žÙÒÙ½Î?ˆÒ(x6v?‡µIb†¬?¬éû#$ÜÔ?›— þºF?ï4'1¬†—?|•È"öÔx?qkÞS¿'?g!ù(è-?•Â9ßÇ?x\ÆS…¾é?ìÛg¶·P~?¼zúöß?Š[••ñ?"$·""?µÙO–ÈW?ºú蜔©?íè4Ý5Ù?ºÇt;nɕ?GLjè?–áÿ7Mâ?­*Ó2)Žh?¹‰¡î(œi?ìWv‹™óÿ?§1"éù²?—u‰aË?'Ìág3?·fé:üJ?¥qv!â‡?íUHwÏ*±?Ÿb([lL?‡2ô¸½åî?ƒîÀŠ,?²o]¬&»¶?œŽ(ùÓ¨ûAGN4FGL J1212.7-1402?ï»|8Æ×&@Gã1üÒNÀ;lk§îÆóÀ<¦®òÇ2Y@ ߪG;Ô?ÿø¶zzða?Í&"©x3î?^ô¼kZàÚ?ý©t"$à_?ïŽ:ºæñ¿Ö¾"š´¡³¿ïÐéÅ?áý'aĖ¿ãˆŸvRl´¿ÞØ⚔kAGNbcu1RXS J121240.3-140141?ï€D|—çN?žé
JO½)?j+s0"CO?Á]V='?‰dÿv¿»?™Ùάº¢m?ïÂqÛÿ3–?vÒå«A?Pp˜ùž'†?Xk-â¸?zªë£Ây?s˚ԟWˆ?î†Ä?_'`?˜ÞV·ò ?c¼kCÛx?ckÙVðÀ?¦WõSax?—Ó4bì?ï{$á-Nd?wõ¾¯dôW?jz
9ç?^ŽÛú?Š±é
‰àƒ?u…àOn§?ïŒ+€r'U?˜0•¢}¾©?p.¦Ç'˜?˜÷äüº?"Ý̊˜Ûë?'sT!c?ï\©Q±V?'!fƒÌæ"?_<KJÚ+t?fõåàÈï?'w€Ä<"?g½%%Xž?î\Â
¦ ?–"Ú¸µÎ
?f«ÇõD¶£?b-beô?¨É!¥W›?–aïµå<¡?î<½ŠÝó?™ŠÒzo'?‹ð9µï•Ä?ˆÖDew¸z?¥8·B†i?•^ä
,ÞîAGN4FGL J1213.0+5129?цˆÈï{+@P%˜Çâ'AÀ:jQ•ôÉkÀ<°!èˆ6@aþ÷KÑ@pÛ4n?·<? |LW¿–¢÷Äг?Ú¤ÐÚN@ýŽøUç"?ïDž/IŒ¿æq*_Oð¿äÊìB3]¿ÙûÏdÛr¿ã@TN5íù¿Ù"-Qqâ›AGNbll3FGL J1212.6+51351RXS J121301.8+512942?ïÏú<­Á€?lÍ‹AKT?S#´Ì65,?DL"©ªéº?s9ô[D¾Þ?j±qÅɲ?ïÉCÕup?w<[‹!ä?Nù<â¤@?TàuØÀ')?w 6ˆ©Œ?t6t†9Àk?ït"²S>?ÚZì?hœÅT$ÈÌ?o0yá=«?Œ´	µÊøm?y°Óƈßf?ï™Í¿Ì?b"f`œvè?u§±ëŽ³?UüÉRcŒ?}Èg´k?[IŠ=&@L?ïšœÿM?{°A«åÚ7?de%²Ï–?YšTMêW?"`Ïz[x½?w§°eCT?ï`;퉎?uþYó?bL+˜-_"?i4nù[@Û?'¯¬µmD?‹¢ÁÏÐt?ïe•''a?†è[CËñ?tÃþúsÝs?tà…¬sÜ1?š'M¢ (?…>áWÂ`m?îËA[XÚü?€oz©éø?>ʬfCå?sâwQ×c?–Y	ßçV?xŸqÚ>ΓAGN4FGL J1213.3-2618¿ï&‡]yOD@Aãƒ'gMÀ:gn³<À<U£Ô…þ²@!(GœÌª?ùmóXQЭ?È÷V¹Eë?ÌÁïy%µ@@~$É
%@ÿ¤åÄ¿ïÿî' Ç?ïÿÑa\w¿ÝÇyB=?)*sqäT¿á…¤O\_¿Ù+¡ƒóÀAGNbll3FGL J1213.1-2619RBS 1080?ïÀ03úXv?o¸kñyÚ?U˜´…Åߘ?Ev`'$N?z¸ábLþ?lç"ƒÞ?ïËÄ x<õ?w±u=LÇC?Tã³ÿÛqÈ?^{Â?tå؈P÷?qkb½ý¤?ïr{æË?iBÀ˜+È?pZð­?rÎ"^6§?˜zô"œA°?ŒOg€É'?î"K‹'ª?}g¶¦Ò]¢?€JÝ©%ï!?bâ2àÔç?¢¨Ù5í¡?{g	øôíV?ï"OüS`?ƒîàu±•?h¿^yÛØ?`"–båF?ˆè.£ö?Tøu24B?ïsž‰9ò?Ì	~:	ê?g$&¨C×?}¤õ—ðÜ?pN¦éÿ²?‡ËĸKùb?î#…À§X?™4Diâ'ð?8n\Œ?€ªob3ö?©€GÅ×_?–JóFÈ·?촒^\?•±óG®í?MÉ ?Lj?|¿¬?¶GüûHA?"ëÀΐAGN4FGL J1213.6+1306?ËïØñÚ^—@R[Ÿ@¢‡À9·ð†nDÀ<.z>å@mï@Ec#»Æë?¶oè›4y?Èì$+@Ž;—…Ã?û,;rFïS¿º)ß!Ž5¿à_¾ÿ"°¿ãΈŽ¯Z̿ꮊ!V'Ý¿ç"ñÿ·/Ø¿ïþàEO•jAGNfsrq3FGL J1213.7+13064C +13.46?ì˜hׄá§?·éÀ$R?¤•‡à5i¬? üŽµÓS?°ñõRtcw?´'©»CÆ%?äï³d˜?Í%W¾1\?ÐRžw>?ÉÈs«É?¸2G"?òÇ?°Þš42m?陯Ձb|?®á%kå?ºÕY'‡Es?§Oˬ¥+?¸]'Àÿ³+?¢öÔ@á&?èÜ-Ol`?¥
¯¡?Âù×Fù8¼?¤	9tÙñ?³*éo'+‰?…pL+BG?çÚñ³ê†O?Á)`äÐ?ºžbD?³¶¥Iú?º?ËéÿHÜ#?¹/ì6àÂ?ÜՌRÍò?ÐÛùæ`r?Ú̂谶Ÿ?ÐM²UI«?ÂcOÓ5`?º•Œn¸Å?åNΈþZ¨?²ßä*o;ã?dž[ŽÇ³?°g´0ëýŒ?Ã>jM?'¬?©ãñ"râL?âóŸü¹?´	a}?ÒQ¼
•rv?¶\¿|4â?ÃH¹h}(0?¥}9ùŒM AGN4FGL J1213.7+6423¿ç*PÕ@J9C¬ÅÀ:¿ØCùTÀ<ȍÿ1£ç@3ʗé@K@Y|´†…?¹:üUP"m¿±™Ö?è"i?ö'ÄãÊ?T@
«‡WÎ?áM̧
£¿êŠ~¬-p¿áÌs`ŸÒï¿äÏ:eV›î¿íOÐÂû'³?à$"3ÿAGNbllNVSS J121348+642524?ïààa÷cF?…χÝǀd?Qm—‹ä›?d‹P
tÛ?fhÒpª9?øÝb£cŸ?ïÆm	˜°?uºég£´?O&Ÿþ†FZ?SšH{|?xä§"…ôF?rI¦Îy3?ï>^]ê}?j¬ü_Òó?v}wŽÿ¥#?(\çér?'"Öa,2?ŒI›RÌî•?ïá~9Ž8Š?L[6ø.¹H?VCџÈh?=s™[û?c_Ý£CBs?G´':v?ï™SýÇÛ:?'¸©ÎFÔ¹?n[ÿrðš?rÔÁ,ïn?'<E[U?Ž½'`u"?ïOŽm8	(?™o8¸|_?`K?l+l?hüVº»??"Êpû5ƒ?˜*ml¯?î ³HŽ±?™X՘É/?wSåm ?}ç]¦..?£
NËZªó?—®™ð|`k?ïŠLÀU£©?s¾®R˜@?u9ü¼ß<?c*
l:•ò?'Ïцd$?n¯å1à—AGN4FGL J1213.8-4345?ìlL¯!&@2—àXšËÉÀ:Jr}ËÞÀ<%)Wèb@ÚøžaÕ]@¹cc}?Ä[ãÁn?±Ó)]F'?î0kؖ/?ú¶[
í©f?ïðØïÿ¿éÄÌîZ¼¿á6sŸ_l¿ä‹«šM¿àb‹"¿ïÿýawAGNbllPMN J1213-4343?ï7z냜,?8~W¼?a†¸ážn'?S²sc†®w?–ßË{?Ƨ?Œå—i«¥?îÂqIn^?œéͪ‹ô?'ía³ŸbZ?"ñ!"¶úƒ?ž;%ùlpŸ?™9Éáq/Ô?îŸOîw8é?'G€*u?€Ó"üÄR?|àò0MŽ?¡Ö8–«oÞ?T.-ú_
?ìŠW7Rb?grCÙ?–¼*ïì^?u='Ü?µþ;ˆ˜õ˜?ü3†"ò?îv˜såç?¤W<º¶îÁ?w")Ä|Í­?iå<r?¬Æ?ðZ?£ð£–Ê?ì%…5?³â¯Üé~?—Рð9´8?90
Í?µ£—‡uÊ?±N®и1?ìñƒû͖K? ÜŸ ì4¡?Ïß@¢¾?† Æ†"«?´yä3ÐúÊ?£Ü!?çU—4<e?£ké-ç«?ªу>.?k'S-®Í?Ì&ÛzÔK`?£ØÜð+AGN4FGL J1214.6-1926¿àIÆÖqCî@EJ8Ÿƒ¾fÀ;;÷'À=¢ÌHB@ài4!Ö@€\FQóé?ؼ‰ˆª^
?ïÿõ^'@ÌiegÊ?ù…hŒ,¿ïšÇ‰W'?ã¨	3…hŠ¿Ö‹¥»ç¿îD´š¦ßÓ¿èB½—¥¤¿ïÃㄟ6'AGNbcu3FGL J1215.9-1926PKS B1211-190?ë‹D0q?¿œÈsÝÙv?º—kcr¸|?¼aùs°?©¨töô~ó?¤ùIݍ	?ØÞÖ^4Øi?ÐC­`Ã0¹?à	™g«Æÿ?Ðx¤-¾¡ˆ?¼7ÛE'ãl?¸8_ëýó?狲'•?²D§Ÿ¢º?Æqéô?°ƒdïóâH?»C}
?¢£R2°_?Üö+01?³ÇðvÎ}!?ßZý·¦J?´>…žÀ?­vº «q?"‹bXÁ‹q?æ^úkäý?Æô ŒŽ)Š?˕ÌhŠ?Å~4°®+?µÞ,ö?²æ8EU:?̞–p¢Þ?Í<5Om&?ä5"jÍ9?у¢é?‹+¾[=?½8.ÉÛÅ}?ãëOè±Àé?µTG‡>}]?ÏÖÑC»'?³l<Þ<=?Á4é‹õA5?¦¹mî %?ʍµˆ–»?²r‡ÔA­—?åÑ fðØx?¹¼J‰4?¼W'·MÇ?«\TòN%MMIXED4FGL J1215.0+1656¿æM˜Åfڈ@S2œ#·•-À9x™sÙìpÀ<C?»òn@ÿ¿¼îÞE@!	!ç±U?®ôA¡?Ÿ|æ
C?êêú~Ù@'³{"†¿Ð/Ú¹š¿ã ^l¢¿å-¿öût€¿æ,£ÌùBw¿é•}
Ú7¿Ôe™¢Rû¥AGNfsrq3FGL J1215.1+1658TXS 1212+171?ïð¾¢O??U¾T·ƒä¢?4º¤
م,?+8ktè*¬?YTD†ÝÌ?Sº¥ˆ³=ë?ïà"l¶·?o"IÉ}-?8D<ð—i£?Cڍò–?lsâu¤G?l"Ò>Œ'Î?ï­lŽõi?w'‰ÕØïX?X|bQ…åý?XòÚö)Á0?•P6‰¶ñ?v ýÈ5˜?ïúµ²m¿»?(Ñ4.ÈTŸ?%-%iàÅ?U>³ý??»è£•åf?$ùÏÓcº­?ï޻̖¾j?d/#<›ÀÔ?EEœÕûû'?<6ÿ"žò¬?kòÌ"q[Å?bJ´š®Ç?ïœòü?Œ7«~M¬¿?P¿Jí\äÛ?]!öOË÷?†âŸ¾
?ŠÖ\Å26¤?ïHÉå;Ù?Ž'*_{ÅÜ?gY.òh1'?hq;œXO?"@욢¢?ŒŸ~ØDœŠ?ïñ
‰ã?L·|ÓcUº??ÓÒ‡3å?151u·"{?UöàÜv%ˆ?GmÀà&pAGN4FGL J1215.1+5002?åLéâ 4î@PƒcÜHjÓÀ:†…ÀŸÀ<sŠƒ| ã@ !¬zúÝ?ütA…ÜMs?¹ß>>?³kAþŽL?úâ$íö@@	f†ã¿ë…e?IìÞ¿×f'|E˼¿à.jáö)½¿Ù~˜¡ÌîׅܿÜz>à¿è~ú1‰æAGNbll3FGL J1215.0+5002IVS B1212+503?ïÄȐ–Õ^?khì3_Ÿî?PiGÝ[Z°?<X,]j…M?yeԛÒG?i'Ü-k\À?ïÀâ˜æì3?{ä×]S?TԈàf@'?]²wWþ?zY'4ÓîÀ?wÝÈÀ?ïo…€?{À
{…ˆÉ?goÂoûŠU?f"umjf¦?Ž?îÚuR?wï1Èu?îþºÔ'#?u\­~ "b?'ëS1í™?c÷úÎ3B?—g/Õ~ÎÇ?qé7$þå?ï–àd·Ã.?x¸(ªý?cL† *è?Sæ_Œ—"?…tÅ8~­¢?v}ðžË¡?ï,Ñ3±)Ñ?"ð$t7¾?oz—Ò@ht?u°è}Þ¤?–v†–ëØ?'µ\Ñc˲?ï5;€?…ä!'S?nÂn4öÈ?ez—T~µ"?š¡±NS?ƒ¿UY½zc?퀲¢©R?'ºýY–ü?"Ð…^¼2}?%¦\ò7?®œC㜬?á½8žñ·AGN4FGL J1215.1+0731?Û±·UŸÍC@Q%¼¾aÏÿÀ:œ¥ÛÇ;"À<k
€òç@!OŽ%óÃ?û/ã7r]?¾9 PB
?˜0':±š?Ý-o|@5ÜiM¿ï¥˜Æï¾?ïã€}"Ô‰¿ÝXcg™¿Æð»ix¸¿äw,ò§Q鿾yĒÁ³AGNbll1ES 1212+078?ïçÜ´ì?Rm²ÐLÂ?@Êræ÷1í?,ªo}Ó?d¾†—ðf?Pg¬ËUQ?ïÓqÏ{'é?uR£K+6?LCqܨu$?S±«L49?r¾ªõØ?qñ+£]Aî?E?­É?pÁ†F¥[½?[ºØõú??Aç}'—°?ˆowGTª?oýðS`4~?ï<Ÿ
x?pN¢'OëÆ?vòMÔåñ?Yß>?'¯ŠÚ‹þ?lÓS&~&?ïÙ"/¶?`ºè¶ª?LwêÀ~~?=(àÊ'?o¿Ö2¾Ñ‡?]*H	 h•?8Ìû?‰š©þ°c?U'ˆú—Z?a…#I=?Šë`Àòêg?‡øëÎ? ?ï#qV%óÒ?$ÞD‰?eûÁ£—(	?Z»§4ޖ:?˜Ò]	ºK½?€>'§¬ë¨?î0?˜öñ?‰l}mP<?‰­²]éGà?s…,d3ô‹?¦–°nò?†¹p?&]AAGN4FGL J1215.1+3513?ވCœs#õ@S³Q¬šþÀ:׶6ˆRIÀ<–µI"ˆÁ@Îbÿÿ'@<ewS?Æ¢
S?ºÝzÐj?ð#	"ãÿï@lÿGµ¡?ïýl!'J@¿äž‹`Æ¿B¿èúàŽµ:¿ä îzÔ]¿ïø½KO‰«?éÓÈ3àØAGNbll7C 1212+3524?ï³üÊt
œ?w
žq˜:H?\õèFrL›?U7"çˆøP?~Ä ¶mâŸ?t¾æ弯·?ï8Ý³N÷?•ï5æ"l?v\†ÿé"Ò?|dbýîu?"V‰›Ø`?'7¼®©$?ï	ãÈU³?Šßù¸-Òx?wééó¹?qøÿm¤l]?—XI#¶A?ˆÌvËd1?ï^eé"×ä?tTƒÃÏ?…,«21ü3?lð ØËZG?ƒ9ÚoVÚ?eƒ›˜†Ðè?ïm×eúR8?ˆ½¹MWæ`?n¾­°íë ?i8RQe‰?ŒÚ{`ƒ?†K'—Ð=[?îÏ´ø^?­' 0€?…ƶ€?'Ä5¦4o?©aW)yÏc?ªA‰E
7?î4ç1–¿¹?–G¬š…ÛT?ˆQ—h™ˆ?"Ú¹°¡"0?¦'#͓?'šô¿y?í¹H¸¢ëŸ?–«ió=?¢¼»išoÐ?jñì

?¡®¹ʋ9?‡þå]ØAGN4FGL J1215.8-3732?ïµD@æû@8ˎ\NµpÀ:ØxFÜÀ<h)à¤&@o›Cgß@Ö¢óµo?ȕè41_ô?²
M`Ûâê?ë%ˆ M?þùr奶³?ïÝÐË_ƒ¿åä¶Î]Ç¿é®`Ðû0¿Ýgzbœ­J¿ÓK' Q¿ïþÜIA'rAGNbcuPMN J1216-3734?ïAqò-%õ?ŽÎlÈ¿?YšÔÎÂ$?PIÇYÁ»Þ?–8qæ?ìåÆî¼a?ïÏÜT\×?ƒ°ê`¶ð?gjœés¹?iaœNih?‰ÄîU4o0?€.z,½ƒ?ï'‰43õ?‡>òû'6?k*ow ?c™ÀƒÜϔ?—©™#Ï~]?…{;ÃL0à?ï!l¨¹‹ì?uFò«JEo?pÙųåµ?WG
ú[‡?—œ%3B?sqÙQ¹‡Ö?î|TLnª? 	c2Ø®þ?hÈr~w¡?e.ˆ¨':?¦²c'gk?žÝqͲ+à?î×9ҁ*?ž'q 86?u¸úÈ1¬?€Ÿ•rÊ£)?ŸÒw[zQ?šYþN$%N?î16d¿a?˜ZׇZt?wbÚ	ˆ)Y?rÜŽW)?ª>y™fF?–Ø:ã>?íQõêcœÄ?'óƒŸJ ?‡ÊVýr?wû¢m©?²wν¿?'»Ìy¸AGN4FGL J1215.8-1733¿ÚKDc©•@F=Â;yRÒÀ:F¼—Ëc@À<H…7È@N´©‹Ó@ú0bžZÉ?ÂÛy¸Ó›ž?³Ffdÿ´?uøª¡@—EôÖ×?ïiæþÒ-Š¿ãã
ìQÍR¿æDڐå×ê7@Þí¿ïÿèþ†®/¿íÈÔàl'ÏAGNbcuPKS 1213-17?ï—øþ¼ª?y#5>z?müödsÝ?_ñƒ\3¼)?''ƒŽc?t«6ü‰5?ï^ÉÝaÎ?‹å¼r1(?s"u¸©Ø>?y§iL0ƒ?ŽƒMº¹s?'¢
*eÒ=?ï9ºœ|*¦?"U§'¨Ù-?xLcW֒1?tg_ͪt1?'µ" 0a?õœµ'÷?î«à™èÏ?~Ë ;š	?",VÏÅ{?t®£yfÓ/?—W\ª&§?q#cpb•?îñuuøՔ?4?À?""Àïsëµ?xŸµÁ†0P?—ŽðÅ»»¡?‹¼ÁÕâp?îEéhäÅè?¤ìõŸ"?†ãîi?Z'¡/ð?¦¥wÜ  ? ß6†È?îUOìb¥x?"¦xsZõØ?‰i[}?'V"?¤K&âöb{?ŽU@zù®?ì0/PX;?–~«Ä£åK?¨ï»¨ ë¿?f剩"?¯Ad'^"?Œ•m³RAGN4FGL J1216.1-0242¿îõÚx9«%@M{›€#¦ÎÀ; ÆÞvB|À<›'–FþÂ@ Ëÿ)@k*?þobð ?É'dÈ×tÆ?´¾¾l6à?îcâÞ1#9@Y‡¼ÍPU¿ïÿZ=¹?ïêâ—9m	¿¦IøŸ¿ä|â((¾¿ÄŒùM3e¿â=)¡dPAGNbll1RXS J121603.6-024302?ïÃd8Lh?'‰­pïŠ?XëK=Å D?È‡¨1`@?xZ G?eíÌÀ›7À?ïÍ%¼ðX?sâ™Àkx?I0<.äÐ?PzÆ¥Uat?vGv©6?p Tö[ÏO?ï\Sfj©R?#§çJ?aÖ%>ê}¸?^üb÷§?':Ήţÿ?}Ô«]ÒFF?ïM‡Æ™" ?sŒš/ԏ?bϟ;wUô?PŸð#R»E?"õEŠ¬I?r¢™ÓXü?ï‡4–ym?DŸÀQ?U6}ÞZ?HÔÔ¯š²?‹Ž''$Ü?~Kȳ<Ü?ïhX7,E?Ž"jóoÍ
?XyÚ»è˜ï?a:Ž{î5?'w·F¨°ä?‹ûrCíª8?îÉV¨®4†?Œ=ƬnªÐ?jb'—…?brÉÔ¨kø?¡ÉƒÞo­$?ŠÍ"Ôä7?î{WAä?'ƒYï¾?sф?ˆâ­?iƒËp#?­5GƤOç?'D×ÄyLAGN4FGL J1216.1+0930?ìh-èèٕ@Q Õ{Ç÷{À:bSåZbÀ<|ërl.@ndD"D@#~Ýx?¼aU"9]?ªþ8C'$¢?ð×*à¼?ÿ†k5X'¿ïð'Úb·…?ïS(Ü¿Þ¨»àì>'¿ã™Á§Õœ¿äƒ×ûÔø¿¾éÀÎfÕÍAGNbllTXS 1213+097?ïË«*_ü?i,•¨Ôæ?Sú%rŸ?B‰Á‰°#£?uglJÖèÚ?foWiÞìæ?ﯩÕ=ñ?'MÛy9²?a—3vn®?kw½f~?_¥h˜?zWƒ0ãØñ?ïmêĄ~Õ?}¤N÷"*?lpO7:?lÞ´P^".?€JóV>õ?wi[™ôÕ?ïekû·Ø?x-ß·'Í?Œ¥aòìÐ?q8ƒæ:BW?#¥þU&?jXýé›9?ïš@;À†ª?vnm·a­N?dz­Ýlï?SþsU:®¢?"QEÉ_b?s»<õ[c·?ïŽúÈøF?™w|:Ü?tKeh¨ù?¨à³UL?˜Û9O–'?"Óžþ&nÑ?ï"™>CÌ?†9ˏú£?uÇ=žøzd?rÍOqáÓr?™{½n=¨á?'O&Ê=R%?íõ,-k¯7?'q|Ðþ8>?…mAëÀ?‰Ee¿ö›?¡ê†"ߐX?"3Ø32(AGN4FGL J1216.2-6121¿îÖèæ͘¾?ó˜2ü¬ŽiÀ9Ü»‰®jÀ;(};•"@•þYŒ¹@͒Z
7'?Ðùn
Áà?Û¯žS<½ö@	¿v¢ôŒ.@ ÂèóI?åmíät‰?¿á}S³{j¿áÓçþ×`ú¿îO
`;¿âzm"gÙ-¿ïà‰B37AGNbcuPMN J1217-6113	?å	.ä[N?Âð)ºÛt?ÙAÄ(`?™ÆP»4?Ô§½É¥?ÂM0ü2|:?Îc	­±\7?Çï½Ì˜ŽF?¥ÏªvÜa]?£å¯ /?ç
Bí$m?ÇÁ՘"v"?ßé$Ü®AF?±úËÓFœC?µD½$Y?¡YòÍWW?ÚÖIó¾ÿ?±¡
ÿ™ô?×V¡(üoõ?¨¹rïµ?ª}¿Ê5Þ?‰‡WÃ]á?â¬Ónì5¸?©ÍTóQ?Õj´¹Ûƒt?¦æ‰6u?¯EGŸá8?«jhôH,c?ãYN|ÃS?ðúò'œ†?½uS5©?¾ºÖU6¾-?ª´ÿWŒÏ?¯vù•.…6?꼑‰[Î?Á"~^¢<?Ñ4j¶YF?±×ÜË:?»rÙU5*?£¦ÒTZ§?ä<IÔ¬·?³Á{–‡"?¿'R©á?‡ÿ–¸8¢?±:c½7?škþÔý_÷?éæ'Ôu¯ý?¢"°a0MIXED4FGL J1217.9+3007?îǍÑB@Tƒ×Ûô‡ýÀ7ÔÄèÒ½À:ÝgD²·x@ýpÌÚ?ýªˆ>•g?'H]+?§¡—s¡k@6ï^Èt@Δ$9Æ?îg¬sßÌ¿Ùù{Óë¿Ýç‹z‰‰¿Þs¨£ø˜-¿áJ'Á¿Þç=[«!AGNBLL3FGL J1217.8+3007B2 1215+30?諾}nj?•"k4+€·?JHI£Ÿx$?V´X"tó?"ô6'l?"ÎX"h?ïŸÖå¼]?‰rÀK{x?Z¶æ/A/¤?gT-ɌŠ?"³ 7	Úß?‡¢2ZËFž?íóí"¶@ø?¢R§:îž?€sõ_Xü)?†`tÃœ?¬¤0~%‰w? ôú§Ÿ=?ïÅËòS¼?eðâ÷ ¦Ï?Pá:gZ%?>€£ÎíC6?ytáÈï1û?dÂʨ¢Ñr?•5°?"÷ñZÃ?H~ó£.;î?P¯Ô€·«Á?+aÝ´‰?"tÒÆÔÑ?ïÏPyƒé?¢J
e$?j¯Zdê)C?{ªÅìKþ?™p*«u¥?¡'Z3"…w?îH#´˜¬?¡'ia¤|û?vµ-á%$?ƒŒñð9º¿?¨¡K#EӔ? iõi(W?ïb¼bÇK?~ýxòD6?\béd¡*?TpQN-?‰óµê"%?~Ë «ÃQAGN4FGL J1218.0-0028¿ëß4¡ÐÓ@NŸa»úìÀ9ûKиê˜À<0=áÄ@b÷Æöt@26 M}a?»®ÌÒ|å?¸`ýµ'?ùhöHÇ/@	i
؅½š¿éã_•'Í?ÁríÒ¹K¿å^ïäÿÉy¿çՍ@öv¿Ú">þî]¿é¹¡KêAGNbll3FGL J1218.0-0029PKS 1215-002?ïá|›YI?a-ý92B÷??/s|€Œ;?1"™Ô?jv§Šö¤?_šÎ¸ãH~?ïՖn…³x?q¬èÊY?F;•¦ìÈÌ?P¨ÇUle?rmUô¡M¨?m˜‰cíkx?ï ÛT¤òé?x€Zî
Æ?^0ŸM]>?Z2s{?"ä1¾?vã¶Jö?ïy<ŋÃv?gä¬Éinm?o>–Ÿ±d%?R±L_b?‰á(ý¹Ï{?eÄyãbÕ?ï¾q›+r¨?rÁòm¹›?Rd~|3³?FÎ('ı>?|.ÚD¦ð?q4RЮïò?ïyÞٝHX?ˆ{Ga"
À?]uԊ´¹?d'æ(\ÐD?Ù~¼¿?…ÍßóûLØ?ïR}OÙS?†ºž$'f-?kO<:Ǔ?né@ªz?'FrÄÝXû?"Yœø†?îsï{?‡|ü&õ?†ÙÓ@eh?sd'8jÂ?£
™Ë"rÖ?…P òÍi4AGN4FGL J1218.5-0119¿ïkšÍm¨ò@N;gäçïÀ8ÞÚVùÀ;©É™;¥È@p¿#¤@-;¢m}²?¨n'>´Ï?¹3©û'†P@À2˜À¥@ÌÒÖüü?ìïÀÛå¿ÜÈ¥ߙX¿áéÄ[å¿áb©B"	¿äës`¿çôþÅwAGNbll3FGL J1218.4-0121PKS 1216-010?ïî"{',?RÁ¼VE?>,¦'GË?3ëtâ˜ó?\/ß;›SÜ?P½_½o?ïҘ —²?qv8J-"ˆ?K'K•¿
‹?R‹>šÁù?sCf[҂O?lÑ©‰|ë?ï³Øcü D?yÂIäÉB?e8Ïõä,Â?rœc[˜¤Ë?{wfL›Ÿ?rr~Æ?ïƒÍ{.°©?jÌKàå›Ã?dÑû§»!?H» üêC?‰Ø[ÿ¸ºû?hõ+'é£?ïàD+†Ÿ?bODÅ܊†?AQaš8™?9Àõ<X,?k\éh&?`ÜV¯›'ã?ïwO'IEï?‰˜×I‹³?a"[—qöc?mµ=ÔÁÍ?Ë‹ñŽ™?†¿aKÁÁÎ?Wwå?mÍøÍ?fÒOa£*?pç¥A?ƒãÖlÉWþ?zGm€ú¤ì?î¾JQnò?ˆ »ú€…?zRüÊëôú?fRw¹ýi±? ÐûO	Ä?†¿
ÂAuÅAGN4FGL J1219.0+4827?á	‰œ@Pñ<64À;d‰èK®TÀ<¾©Ü¡V@àÕ:Y˜"@](¯Fª?ȤvçvF¿Š­ükå›?‰ö­›Ú@išÎM?ï`¤&ó¿æBnd!¿ê¯s?è£B¿Å
GÅwÄ¿ãît½A>¿ïÿf¢¡U%AGNfsrqON 428?調ì­Ü?°ÅðGwÏ?PèZÑ?Nhu~Ýq?ƒ4rÍû¿Š?°ÈnÒº3?ïÑ_¨ ù?txˆœÛL?Aè{[u6`?Gùr5­Ÿn?užc†L?s#¯†¬~?ïN\òtQ6?ƒÙ.–Öš¦?f`ì?fÒ¬S£Ë?"VŒ¾9Ã
?'Ôq'"ž€?ïÐ]"@ûY?Wn¡d<?XôÙ.¥œí?C™4Yí?q"ÿ¯UÌ?SãµôžP?ï'óíÍùH?¬R%Ò! d?b:|î3H?XTćp?†´ePPuD?¬Vr­;?ïw¨³«¶?ëZlã!0?R_e](Wi?Z{ÆXÂÑ?Êê/·'?Œy‰íá?îÆíÀ•åc?!Tš~I?qªÝSúžW?l¬°øa?¡[ÈKà]‹?ë}õ?ï_]zl;?wËÛÃ-9f?uÎðîá
è?f—Ó£!Å?A)c¶.?sî'xüÖ¬AGN4FGL J1219.0+3653?Ûò‹ø
,@S…/D')‰À;oP–À<Îâ*,#t@nx‹¬ñæ@©A­Iz?ÓÀQ>a¹?ÖÇö8Öá#@÷P™u‡l@B8!°º¿çt]î$?îo^‡ŸÇ¿Ù£½l²†¿ã2HQ¨i@¿ïûñH¿ïë6ÊñUAGNbcuNVSS J121915+365718?ï ò·Ê?ð!¶j'?'Ý4}zôý?z‹ªâ"À?'çp}9?…Í–åùÞB?î)ëÓņÕ?°Jۘ?›ã@è¹£‹?¨Ea•éƒ3?žßD›%åâ?™7äZÎ{Ð?íiGú•‡ç?Ÿv‰Öh?žÈA"Ah?'úԔcÇ?ªb7•®Ù?–Bý¯ç»?ì¬e'g1y?–»kÇ"¹?²¶·ûÜF?•|¦¼¿O?Ÿ˜mʈÏÈ?{$ÍRÐOÃ?íëPޔËT?¢‰sHÜnª?–À_"ÿÊÓ?Œó…v¶?¥êÂJû—_?œÉ•@á ?ëïÖg³Ì?¿*¦" UW?ªüâr´$ ?³ñÁ'2ÒM?³ú\?±åA"04a?ëà«Æ=m?¥ß{«;?¦Á,IxÞ¨?˜â{¡Ê?µš¦[±È?ŸvMqm¾?ê3Y›t1£?©Ó!ÚÙ?¼fÀƒý?¨Ê5k?>?±þs®ân?"Ft˲Z+AGN4FGL J1219.0-4827¿àBÁ ô¬»@,#ÿï9_À:+3ªQwÂÀ<>J—ÓƼ@bxqÏ{@¹m	Ö¶?¼jgÒÍõ?ÊULù	ð@âÑ¡GãÄ@ï¾'˜uW¿ì	ì³!Ÿ?Èx¤&æI¿áå¢áìď¿àÆY`nº¿êÁ¿åԐ{æ˜AGNbll3FGL J1218.8-4827PMN J1219-4826?ëà·µZâœ?±¬œ¨ˆ?³hûªÑgv?ªmÕQ3W?«"Q?kX?  ´•ôH'?îMx–<?£‰ŠmVŊ?'•W9å¹?©u2m?¢]ép?¯Î?œÎ¢[Æ6?íé[ñî?¢ˆÀq^aì?§–˜c\Èb?šoÎQÙ§×?¦jÑßJ¾?"óD»_¬?íOTn—7j?'é
\ÎNå?ž«çò9<?tLøÍ{¿?«´Å vD?|-Û=§x?å:ÿÚ¸•*?Á^ð¬·ä?Êü/Þù?½Q΋¶#Š?ÀÑ>²T?¯"âÿôT?ëd	;²?ºr>ï9?¬)‰Õ?³T¬Òå?¶ÊÚȏ° ?±$'dB¶?èz4à˜—Í?³º˜»aæ0?Á±¹º:=?°.®R ?¸Ì/†|òŸ?¡ÎŠëj—…?éPGjš?šÉÂ:Ôe"?²ôDɪR?'…ò:ê?ÁDÀhÓå?"©ôÊ[$AGN4FGL J1219.6+0550?æcÓKcx@PÙ¼¾aÏÿÀ:êÒëʾÖÀ<–"
>@XÜüŸÜ?ÿ'ø½ì_9?˼#.XX?•_¼~?óF«ë«µ%@E9ÜœH?ïÁCâWùf¿ä.y$¯ò¿ßõ]¨)¿à{Áâÿ2¿äL-4ìp׿áÿÅGAGNrdgNGC 4261?ïÏï¦|½?d@͙¿?Lqe'?;J}Thu@?täÛ¨Üÿ\?bҳŭ‡W?ï½²µkԇ?vL× ^?PŸ˜Z?R{Ëq½»m?}½rÚB¢?s¾](¾$ê?ïƒkãäý?v8¤ŒëÏ?Z.½ò°1o?B+¼â|¦œ?‹ß/I…z?uf:·•á?ïJèœi¶?n"qî°#€?uò
¡?SòâYª¬ï?'|n€§Š?l©$«ä?\ç"?vÃAŒb?[Tµéû>¢?MƒÞ£¹d?…rR¾Ð:?uzÁā?ïB1òQ§Ï?ûiïèÇ?`\NïÙ¤?eŽ!"O?•®7Úc˜"?´p'`Û¥?ï—a¹Œ?‡Ð2ž=\?e…3΀+?W_¹_BìË?œœr⬥=?†ï~Yu‡Ú?í÷Û³oT?Š2lÇ{£?ˆX~8˜Œ?q€'Æøˆ¤?ª}®±¢²š?ˆù.l´e AGN4FGL J1219.7-0313?»«Ó\LËÏ@MYµÜyÀ9õÍXãÆäÀ<7"U²¹ü@ Æ2ÿ±§?þL(²¦°Ù?¸DÛ&VÖÑ?§(ÍÂ?ñ
ÿˆ
ûÝ@+«	X™I¿¾¶x¢~¶¿ç
>¢¨!¿Ü'|ÉV¿Ü^-ØÖ¿á(aNcæ¿×	ýDcÝAGNbll3FGL J1219.7-03141RXS J121946.0-031419?ïé¯h?O zŸ~¼;?>?œßuë?(A™ŽcS,?c*)(S?r?L+¦TC R?ïÖû25»?q¼lÎF?DǙ6ÏÞØ?NZ‰€kqH?qéF\³Æ?n|}=ç?ﺑ¨MUb?aú ¦ÁZá?SLœiA\ù?<>-6Ü.ß?}äÝA‡‡?_…÷IÑÆä?ïT\ËTt?iùaдt?k¦*;ßÊ?FJ¶μ"?'×53þ?gº÷G'¼r?ï×ý䶒=?_Õ©05µî?L4ô†½??84+\£d·?pzo.wfÞ?\¥ã¬õ°^?ïxòD"C?ŒJ_d_?W
Úú¹üZ?aÊkÐø?ŽâŸ³ÓÆ?‰¤[ÞZæA?ï}8SK×?xõCÍUüë?]ò½w¤?L¼Ù§üw;?Œó§8/õ¦?w.†rxü?î49ÁJk<?†÷ýÑԖ?€Á£mì¹E?d1LL¸?¨‹ûhHu?…´S#AGN4FGL J1219.7+0444?ï¨,°sa@P˜0O‹YÀ:Ÿ܉Ù2À<rœ…dž@ 0]E«Zâ?þÚÝð,M?Ä˒ûoÍm?½håq´MO?÷ÚÀZ΂¯@—ÎxèI¿ïI$i¢?ïü¿ÙŸC'¿Ð3VćÙÔ¿ß«Ø ër¿ã¨bõ˜ñ¿Îîï¡ãê÷AGNbllNVSS J121945+044621?ïåÊ´µ™?V-Èê,í"?<šœº:—ä?,±¢4K?f¢Ž£"ôƒ?T‡õB}=?ïÄîÉ°?z~m—%כ?T)Ä@¬"?\2¼\¾z*?xdÐþ+?uw3aü?ï"ÂÜ?o{zMç¨?\‹¶P5Vâ?UŒ¸•ŸB]?‡>åŒF?k'ʂnQ'?ïN(yh?t0¯…>º?ƒÆeáxƒß?f{ßÛ+?":£G Ü?nø^f†h?ïÒ>??ol§»øÁ?T$ðIށ9?h¤‡Eól?qפXš¹ë?`{ÃÆlú?ïWtËÙݬ?'g&Š^?gxÌô}©?pˆ¹WÙ?'·c¥È?anóÂt?ï7íÒ«Þì?€=øD[	ø?fèÒØý¢ ?[iÿ`?–%+GQYV?}ª³wÝ s?íç¡u
Ñ­?ŽÂ58óœ?"ßhm%?{¼•þ?§–Zö Ï§?‰‰"0xY2AGN4FGL J1219.9+6056¿ãJÂG¸¦@KãEŒÒ
úÀ:ìdoa'À<͒…©!Í@&ðڞ@VŽà3·?»{ÚÉðO¿´á%Ž?øeLöRØ@ãƒJLÕF?í4VCÙ¿è7…½Äœ'¿ëË!{û¤¿Á›!Äuæ6¿ß؜cÎ[˜¿ïÿõEq#AGNbcu3FGL J1220.3+605587GB 121716.0+611442?ïènVð†?q"÷
)"'?Iî93Ó?B†Ê•¼±.?a¾Ù	h?pŽn½Tä#?ïڂR³´«?n˹cM×?A™¬q4æ?I_é+
?p‹´Eð¹·?jÎUt6ï¼?ïqió'w?‰*
Wœî?a`M5#‹"?j2 ¿`N/?M¥9å_?ˆ6â'Æk©?ïÔÿwU2H?W<4xН?\6A*з¶?E›Ü4;«6?låh,´N?S£î'(•û?ïÑ6™Í¤—?sY°ßR(Ë?]iœì×Nœ?VÀw6gÐ?p
KÎٙ?qF«/£?ï~+°÷ö?ˆ?I<Ä]?VŸ27›.è?\Î<RŽ ?¡-€¤|¸?†SðÁ>fR?îýníÀڞ?'Ž–A†™H?lIæƒÐ*5?rë]ù³ÊB?œÈåq`?t˜S)õ?ïT"ì‹?zZ¥u¯Ï?·	]I Î?pÈuJT?Šÿs~'?tu°:­ÁhAGN4FGL J1220.1+7105?äÉ#tú(@Fèdìé¢ÆÀ8¨Ê^]ƒiÀ;ñY¡\º@R'Ž7»@'a|ÚQ?£9hs³?ÀÃøzût@­'w>$ÿ@ Ú¨Ø{Ø¿Ìe{Yè~¯¿ß?YÐ,¿ãÒú
w·È¿ælfû·›ã¿éÍ•I¨À¿ê7@Iq8AGNfsrq3FGL J1220.2+7105S5 1217+71?ïÔtõ±ƒ¬?iÞíÃì¹?`Ÿ¯ÐÏ?YTRßî4?jëZ?à?n?bÃ	î€ý?ï¾N—'®C?xòlµ.=?QÞÁÔj?]k'ヅÏ?|aØ' ?vs©j`?¯‹jÏ?ŽÁË2í?yŸ6nØw?"õ0[Lê?'Iøé(¬«?ƒ¶)ê)•?ïôèÏãq?@#`#ñ·ä?<ER²ÕCD?+'yðº?N<Þ´[éŸ?7†ýíW?ï"d
Áz?ƒE.V)UX?p'¼gÏ?n#ÓiS­?'Ü;æo:?~/݌¼R2?ï8ä7D?¡"š,pß?aÁ×Ö1Ð?nÙ£ÿ´åª?–«V]ïDR?¡ejÍZ9¨?ïEµÎ¥âJ?'|f•?Ù,ôV0ë?‡ ̐æ?Œ¹_`!x­?	ý4¸6?ïáQ>6›?^Øöýg?R·uW±÷?D8»_swV?e­æMƒÉ?YKª×é8NAGN4FGL J1220.1+3432?ï=™Ï'"·@T»ìª¸¦À9áéÃ}˜²À<pȖg"@°˜a¶(q@l÷¢cl·?´زP\?®¼œVÉw?ù³·‡Á*@	·nN<N?ï"ÊÀ9¿Ü…SÜ¡@¿âÓŠS«¿á¤…†"¿å>þ]hã¿á,1·20ÕAGNbll3FGL J1220.2+3434GB2 1217+348?ïã"ª‹?á®?r΀?AèmÓV?IÇåï˜'ò?h•¶DþíE?~èz)s5?ïÊB
8C?yõ¤žÅ?Mê;Q%p‰?WÏ0ñ	Ñ?w!±û@Ñ?u4-,E?ïÈMŖ޺?dFŠ¨5ûÒ?R}VÑH¶–?S˽2?w9ÇoÀU9?a>Ž…5?ï"ðmeß?fÿ»n£õ/?zøM 4ÿ?^Dª‡ÞO?{~º")»Z?[âÇü©—g?ïá±?Ÿõv?rhèÁ[ê¶?GaêM!‰?KHÿ "~5?hvEìÈ9›?oD-¾½?ïPG+ÉÔ?—Šæ¸C?b҉	‰'©?l™Û·ŒûÒ?"œÉh®"?–?
ÏÓ×?3õù?súËKÛ?Yãñжõ?SÅ3Mü·r?ƒÜõ'Ê÷?rÐŽô?îãHÌøk·?'ÚýÇ«w«?'ɑrŒ?wøÚdjƒÇ?'yÈùޝ?x|(!ã¦ÂAGN4FGL J1220.2-3713?æüA±"Ç@9;·Ç'
1À:?ÐW›ÈHÀ<`«l)ôÆ@ ã(å?þT·Æ«K?ÀÖ3hb??¼,žïnã8?ý©ÙgåÂg?ûkcˆ»zë?ïûG¿1X¾¿àœÊr/ȿޔÒ?R{M¿Þ@)È¿ÜjÈéÕF¿è]'ømåAGNbcu3FGL J1220.1-37152MASS J12201982-3714137?ï".q"§M?ƒ‹ÜºO?W–î†íX?H~Ä\NmŽ?ˆRÄÔrî?ƒCk1њ?ï1ii·?"•"-GV™?€®ôas²ß?'ô(T‰¤l?"ÂX¯¸w¨?Œ²r¦Î`?ïD|B?Šà òW~?rO¼Æ7cò?oñ‹Lì™#?™#J©'¬?ˆ£fðüŒ@?ìåâNƒ	¤?Š'=÷à¶_?1ýÇú&¹?v¬bHxj?±"nÅ0?‡›·Ì¢"ò?ï7cê
J\?ŠP•ð‹Â?oA˜+Pæ?^ˆÄ¡8?•+O¸DŒ?ˆÙ7z{ØO?텑M'?«tdSW9$?—D!|ƒ\Œ?œû–è#[?¬ސ]t"?¢†ý'?î0	šÞh+?™ú­ë.Ç?|N‰~?sƒðӥΘ?©u•"Nz?—÷ðÿìeÃ?è{V¸üéÔ? TÑŒ]?°%WÂ""˜?'Jé}õˆµ?Åÿù:ûæ?ži»ñ	!AGN4FGL J1221.3+3010¿ß'äëôÓ@T¯ke©¨À7ڊèü®<À;/jWWÖ@ Ó]<F,?ú£%"R? B³·[? ³~µßî@ƒy³J@a· D%¿âSÇÝúœ"¿Æ‹sü|ô¿ÜÁ¿àáW¿Ñ†±_ˆý¿Ý—|ˆçš®¿Ã[Â"¹=AGNbll3FGL J1221.3+3010PG 1218+304?ïç—è®C?_ÖÂ"?÷?/Õ^?'°Òý‡º?fjÆ?sá?^æe÷?ï§|´í™1?"ùÉ5,?W"_ {
{?^œ/¢º<˜?ƒ0FÜÔ?'Û·$Eb?î$Ç!ßp? Ý'Ám¦ª?h~^SÂ$Ë?v^oә?¬7ý«é‡«? f…'—"?îk"4ª£ú?‰Eâ@/˜?yá•lEpö?b@¬{õ?¦ªGxÀ?‡Ó¥Æ:j?ïÃJÔ©Sæ?v&1}`?@v\¨8ès?<³$­¥ê\?|KÊsòñ?ugCc¤?ï;žº¸?¡fÝΊŽ¥?iTå™E?}
™oùõ;?™.ðö	Î? ºÞCð+?í£CÖ2jû?¡ó¡ˆ1"‹?r'8õ'3?€q-ý"É«?±½½¿‡´?¡R"é´í'?ì±8h"õ?¡lÿy¾µ?‹¥&8Ћ?z$·C€c?·hpI? ³ðÛY^AGN4FGL J1221.5+2814?éС@Š'H@TÒ//˜tÀ8%\±À;¶i©çÅw@ò®¸dµâ@A(¿<?—`°Þžu:?•š'Ç!?ú/<-­¸@çuXǗY¿Ý—m$E¯¿à¼J~Sm¿ãGüMÃØ2¿àvÚ݆®Z¿æþ\'ÑN¿â°–5a
ÝAGNbll3FGL J1221.4+2814W Comae?ïî4AŒM'?oëà¤J?)‰î$¼?$þd=z–?`3©sðR?nς†šõÍ?ï² Bâõû?†Ò®¼€T?Q|>î"ù?X‹eo¯(?HgbèÀ?…•M¡Ì؆?ïœtªÌÇÄ?ƒS^Îâë?YhD"Þäœ?f{c[|J?…µÌ·Œ]?'"iáZ?ï÷¸<‹»N?9%¯·Ø(?5A˜—4;P?%ÀÐd/l?F~A3	:?2pà¢H"?ïãQ­‹'Ä?c,*®þ™?3o«	ÂÒ?-f'aÔÒV?j@\æˋ?b~Öô:ÉX?ï-="JW½?¤4.'_ÆX?aSÁrÏt?r~ñ÷xwÙ?˜4Ñ8¯Xz?£SV¿)v?ïfÔj¥æ.?ˆ›Ý¡u?cRÙ¬€
?pkSßEãI?»1DØ1?‡4ÝÌ1C?ïîÌùUs?Q—ã>±Ê?G£. B>Ó?@ÅJÁ*?V"v"ˆõ?IJ@öèØ?AGN4FGL J1222.0-4121¿Â¹¤"ŒË@5+ç:6\³À;R[LVñÀ<žË'±ñ@Û®Š—s$?þ鬆Ü'´?ع¶…Ä´?Ó¾-b8Ú<?ùÕt;;?@äïp¶Ç¿íjΪó^?îž8£NN¿â/0¤ãy·¿Ùzˆ|Ê=¿ìNOÿFǐ¿ïÃn_E°AGNbcuPKS 1219-411?ïP•ÝU
×?ƒ¤ëŒ"Î?~œþÀþ?pÓLñâ¸?ŒŒ	"ýsK?}ñ=þfðs?ï´Qµ÷•›?ÿÜ5¡Õ¯?_ÆQ—O"	?iåX°­sÌ?}吂äŠO?x¨¢lC?îŲoå|W?'Ố•šE?"Äúr+Ô`?~«è\Å?œç4Ȃ¼é?…D©ÑjÙ?îè:¹Ëy?t˹BQ—K?€\g{我?aM'Eé}?šÎñ†‰?r&$æ—Ó?µ	Ã?"×O$L?'7˜'«˜?'v+­1?œ±/.ä?7V¯m?ï³­ìâÂ?—ìùZLç4?rÖ<bàã™?{º'6¢Â ?˜Sû&gÍä?"&í¶lÝ?í،>ùKA?›QàمS?ŒÃl̓^?…RÓÔ¬SÖ?«F`Þ"pÔ?—D?‡ðÈ×?홎r…>Õ?'Në_xÐ?ˆ‰7åõh?}ÐIµ|ã?°"j$kW-?ŽäÉDyyAGN4FGL J1222.5+0414¿áL²P¨A±@P…à`þG™À8©åÂg=À;ÁR4€:M@`5C-Ò @{íx:¤?ª	*\[0ä?¸ªê¤ÏÛ@¥åNë @R'{ÅÉ"¿Ù€	e.'õ¿å‰>7s3Ô¿ê$úö«Ãh¿ë©%þ—J¿î]¦Ùóü¼¿ïô[¼¿8AGNfsrq3FGL J1222.4+04144C +04.42?ïóY'
P?Jûµæ·"?7I,ê"ÙÙ?,ʋåǙ?T4	QJ?Gu¡¨o?ï«@–Ú2Í?†'¤½AÇÿ?`ÌOhŽÚÝ?sí1=Z ?€üÆzNUô?€‹J}ÿï?ïpw,9øR?‹ôì(Î$?o—ȄÏ?vŠŠƒŒG
?‹üt|¡Ä?‡â;²Þi?ïÚ3DGz	?U2QxÑ?`ïsÙ×"l?Jä‡Nk?dÝG²³ÔS?J¨ÕœÑŒ0?ïèå=HØ?\F"hPœ‰?Aª&¯®?7^kx¯S?b°9Q°ûÏ?YÚ£¿Ø0¥?ït\7'M? íÖù³?s2ˆ€l?†µRA¥Ä?—ä홺Àu?œøˆ?îó"×ì‰?•ŠÈíÛjh?x ÕÜï›`?~šAUC?›"o®Å—þ?"Éð¹	?ï˜L§?w=ƒR_:O?yœÕ3.ÈÄ?páÅüP?z\yÀ˜?i@b2߂/AGN4FGL J1223.0+1100¿ì8W«žºý@R#ƒQX¸(À:èâ©­ãÓÀ<'Üo×ÿ0@çQÛiô?ü¢\¶º<?ϲ'´¤ã?̯ÀâÞ±ý?þæ"/•ð@8Ca©"7¿íœºëù¸¾?¯Þcß3½Ù¿çÖåŠ2ôI¿ÂÀbX¯o¿â¡¬ÃB	¿í"M!ÆÏ2AGNbcuSDSS J122307.24+110038.2?ï×má@2†?d¾îJE?Iˆ^ŸK?7'H¿?q£>Ü#?bšÏ°Ÿ&?ïÐÆ´"×k?t<¥ƒö?K¯D¦Ã?UWˆn£Gª?t&½/Öm?pÊðñ^‹?ïxòw"Ü?w¹Ô[DJ?e˜îÖd^¥?a.ûT"Œ?Œ]&sG¥z?t²×Ú݈?ï
ò
Ãl?u'ùíˆÙT?x0õåû•?^Ýå=UÌ?˜›LCœÚ8?s0Í£Çzê?ï»Ãè%ã?qA&#÷Ê0?TÊc"=u¯?D[á•.²Ø?|ës,z¸Õ?oÛ©lGg?ïkí6Ø6ì?¹B÷äb?`lÏÐÒÝ?hm]£·Ú?t¿,–°?Œ±{XSÉ?îø—¡¥_S?‡3¡cÆ ?s/ÚLâèµ?k[ðî¡}#?œ!2óñu?…… 퉦?ísäÿ¬ä?"GlK
âš?ŠTÓ#Ѐ?x†$¡'áò?±=¢*•]?'FÕûxAGN4FGL J1223.3+1213?Òçs刎@Rm®ˆ*ÜÀ:Ü<I\jdÀ<d É8Ö@ãw¾RŒ@é§;BÌ-?Í]f"â?¸†›:…?à±¢z¾¸@ámÛhò¿È–œd$AÔ¿å"«=0¿êî±##·¿ÕO*u¿ï¦Òœðf/?íI'w"AGNbll3FGL J1223.2+1215MG1 J122332+1208?Î4'?—÷°_Ãõ?^a;M˜Ã?fÃí|P?ˆO%'"…?•ú¤òç^?CšM?†á,¢—¼l?_·©®žf?eâ.T¯`?"‰^ïìºè?ƒŽì4 º?ï·ÎªÀ?ŒæIÍ2á?sñ1ë¾_?n¯ÎÌm·­?˜ÂÉ阊{?‰¶Åad-?ï®ú¾!¹?f…+b˜b?e$…²dŸ?OwtùT‡?~bû?)u??bKÈ­Ðä?ï>Œï«ã¸?'§2ݘ?jÃRn¡Œ?f\Úv+žö?"Õ÷šÝ?¯S,\[I?ï'lyzë?œF¬M*Ÿ?pâ!ªk?'»a™è¿?™HŠ¶¼e?™)€]ܟÁ?îI_Íù{4?•I´Ê?¡½Õ(^?uÈW)U'?§uËj>e«?"ÖH(]?îî=¡\lÏ?Šukú=`?€éú "µ‰?rÀñ' v?™ÃNˆtb?†"…ÈMÙAGN4FGL J1223.5+0818?í
ÍÈd!,@Qƒ±mÀ:Å@ªÀ3À<Šéåˆ@ ׬NÓ?ý–:iˆYÖ?ÃЎã³F?·¨˜:	?õÕêî ¬@	nÀ
òwV¿ïû5•äs?ïÿ¢bô¿Ù·?œÎ€¿Û@G¿é=A^Å\?"ÄÃhõãAGNbll3FGL J1223.3+0818SDSS J122327.49+082030.4?ïóµó}¡Ó?H¥¦	1"?7j½¾vh?.†ˆ‰,!ª?R¹i[òÒ?DÍ
";zT?ïÞÐíÂ×?qP).—?B«Â#¬?OÜĝ­!ã?l""dƒ{?l埆(+?ï­]ò,5q?wíî%´.?`iYُѸ?iUQdýRÍ?€Ž-	åeW?s"Œ¼«àK?ï·uWùnÊ?_ ÉFÙûÙ?d8£ìã?Iùû¤C{?z)('ô?Yt‡¥?ïæ§Ý\ņ?]pý"×Àô?PFeþLp?G
H´Ý?aRqTÌû?Wp1B! ?ï":%¯€Ð?‡IJ+±Ú?UðÜ+¦€??cˆ9Ö(«Ç?ˆ3Zý$ùø?"¯--l?ïl%‰–0?"yÏ`c4³?m˜÷öÚ±ú?vC–AN?_Ÿ|üc?iÍmÃ?ïQ<mš?y.Ó6ý!é?t¥¢Z7?bW/™¥ú?´ÕŠV?uc0ŽG<AGN4FGL J1223.6-3032?êä¸oóƒ@?ò'B³÷À:Ìsí7¦_À<~ã¬bå@!âv"° š?ù"»¶úÓp?РS\žfˆ?¶çxŸ£ô¼?áqºøŽòw?üHÈK2ÙF?ïýœ"Šï]¿á¹ddIV¿í½÷|£¿?á[æ°£¡Z¿à-ä>ÙZ¿Ñ"î¬ñe3AGNbll3FGL J1223.3-3028NVSS J122337-303246?}OÑ?«ÍÃQ'þ?KŸK:Ñ|–?FæqºSÚà?§€ÜC9?«¿'[ú«?ﳖˆ «?é:s[|?X°>Þx?`ّù1š°?€UòÊ;9?z"–zØE?î>".Ëfé?šo
;ýŽ	?sBÜk¡ÉÊ?y×هN ?©µŠ6ظ?™š'#>ڗ?îÎ æÄ3?"ÓxùÁ—?uŠ}¿—ÞÅ?f¡@.pb? l¡Øœ'­?"tÞ~Æõ?î87ÎðµØ?¦|™yP]l?TÅNªè3v?P¸†åO	?«ÖX›/ml?¦V´ ;[a?ï:X>ì‹?™j訶È?d¤ûÀ´ÊO?q@¤®H?– X¨E.?—4Ц§ó?í˜øÐÇêK?Ÿ"F¥ £s?x:oiþ¢?|=‹û›I?±´''†Õ?Ñp¯òIÕ?ì­t\?¾S?£	ën×á?Œ¸ð¨ÈV^?ˆ"õîò ?¶ý?	Vö?¢g•1øBAGN4FGL J1223.8+4649¿¾'åÚhœ@Qda¦
EcÀ;ŠRuÚÀ<í±jp·"@QP=/5x@Ç¢ PØ`?É|üÕÔ¿Õ>bŠ?³ÝÝ@bp¸@°"õ¦o?ÝCiv¼¿ç'Õ1\½¿ã§gž¿â1_œÈù¿âdµ—&¿ïýAt>–>AGNbllRX J1223.8+4651?ïÑäüÄaC?sRµÝmÛ?G¤ÖŠ›/*?8U¨<¢5
?tæ×Á¾?r—ïîŠ?ïãS?¡?zìlÒGªH?H»?–š?Lj"Ò…šä?{*çpÐ?N?z!
t½V4?ïh¤ùÊ?z)9ié‹?`¤æ·Ù'?R´kùm?éîŠ{ˆP?yEØnññ9?ïÀyþ?ZÙý=È­?Z†ÍîA²ï??K³ûÏ'ž?yPÉè(Y?ZHávÏ(•?".xc?‰MÂïÕñ?X‹H¶c½?L|©È'g•?Š[­²Ô«?ˆáõ.éî?ïU¹ÚÏk?"ƒ?kùîÜ?VíðGL?_Ÿ5À)?"ÙócÕáu?'ÌǕì–
?îºAžŸ¬?ŽkÓr4N1?n=Ý¡»­?ed•®6	€?¢xHz¢p?]…c¤°?ï,ö(³?}Z=rV%¨?rsNÈ?_S'Ÿ?•ö`º—ûf?|¸33óE\AGN4FGL J1223.8+8039?̅ø…•ß.@B2u¸eÀ9dFøâÕÀ<®=•ŒÅ@^.$*¬§@ð[|þX`?¯¤b ^.ß?ÀE™'7Ð@11eәp@
<Èý	€‡¿Ýe[#'+f¿Ý)Ucߣi¿ã£C_1¿âøû^°¿è9îlȿ캫ݓïaAGNbll3FGL J1222.7+8041S5 1221+80?ïäwÖÑ2?\´öà#C5?VêNÑhú«?Q2'EŒÏû?`¿9½™?P#Þ;®t?ïMˆžl´?–+c؂èœ?{,XíÎg?ƒ¼Ý ÂsQ?«ï'WÂ?ŒµèäîG??5QèÍ?…Rª^ó1d?t´lÈo	?~Sï®8™?€ÐØ}¯?}»Äo1?œ1µ–?xžz¼x-œ?ïäøêAe?kà3PÌà?—>ç{·¡æ?nœWo½Y?ïÂ…mŠ?|k›¼ú?sÑâݳV?pθËén?}LÚ~²&Ê?rN݌ÑH?íØá¤äë?°x°S»+?"0CÊK?QXÓ¤Ùô?¨çM'å7€?¨c´ïJ?î÷îÌPûñ?–<°Üí†u?ŠåG¦*@?‹3â¡"}?"'êUžÃ?õþDJ$?ìî"q!çm?'Ž(4S?¤¤Àÿß?†9c)ï2j?¬q÷ðæ'T?ˆßòAÇ
AGN4FGL J1223.9+7954?Õ˳HRW@B''͖ À;Q,50"À<ãQN§-@!Ç&Š-jò?úâ_:øúR?Ζ[K«$?Â58†">?ñÇ7a–@Qõx'â?ïÊýê¦ý¿ëÒ§7E¿Ó"MA§?J¿Ø݂'™¿¹T÷S3-Õ¿éh¿§J\EAGNbll3FGL J1222.7+7952NVSS J122358+795329?ï»î'¼¨	?s'°Ï¹?HX¤',S>?>>èÁÿTî?~ý¡í'OR?r%¾6¤/^?ï–—ú«?‹}g¼È`?`)æpq^?cObå7²¶?†qࠜ˱?‰MPp?ï4å¡J%?†`³¸ÃoE?Y6­sè›e?UPUìeUZ?—ÏáôŸ?†(p©Ó?ïl5DVÇ?vQû
ê†Â?YË{&Y‹ƒ?CTɜä9°?ÜŸÎsb?v1Dx,oö?ïOÕI0~?ˆøZ(¨[?^—k}7ÊX?Pð<Þ³†?"¥å«Œ?ˆ+ɑÁÏg?ï2"ñ‹aâ?"¿ºè	Cj?açïL_?jM"ÀñX?—~£î-?'="=ÇÒ5?î^>cµS?'{s<-oß?`sØAX"?[WªŒ24?©ÜBüøæ?'?°`]ø?íònœ]?–;´nÚ?qЇEœÕÙ?eÌv^(ÆÈ?®¥¨.}ƒô?–5ÚBÜ<AGN4FGL J1223.9+5000¿à€«6­™´@P¡]N°À9¯£¯À<:ʄóð'@³ªºG@YÀª›?³3Áù_'?ÌÁ³éüÞb@-nÎõ@þû¡v‡Ç¿Ì^ÕùFRu¿à4øÀEªÚ¿ç܃ÄE>οèçüÓû•7¿ìÙ@¿ïÿß´0ÕAGNfsrq3FGL J1224.5+4957SBS 1221+503?ïßïê3:?¯¢îí^Ù?–éÌ&?¨©™c«Û?yÜdn¦W?˜JDbS³ç?>UãXÍ?xÑw³>&?ZÀ'>tò~?ic¦Q
½Ç?{°b‰''?r4ìrŽÐ®?îŸîVy"E?›tcv"SV?šÝ³0
ã?•"!	®ã)?'$'	gÚE?ŒàÌF²D?ïµ4ËlX!?aÖOòÏrq?q¹ûõëeO?Vñ}Zš'?s«ž9˂'?V½Ÿy'Â:?îÙ•DE?–‰ˆ•tÎ?›ÅÀÂg?'XݸB×?'-YDò?…Oó
㮝?ï;bÑK?•œ7k—¡É?s*lÕ?":®tk‰?"̵E‰±v?'o'¢2?íý–ç–/_?¡é]¡ý³x?¤å¼­¦ß?–¸ùØ´ç?¡T¥²?™A娐ØU?ïJ¸¾€Œ?"]":RW?h·ÿ4e?y¼ƒUîʨ?Ä™Æ'Ô'?y1	~ÙÔAGN4FGL J1224.1+2239¿äiÛȚõ@T—W'ŽžÀ;^ÆùN5À<¨§<‹Â@"p~]?ÿßCÇÕí?½Ð­¬ö¿"ãL@€?ýáçÌ,"Ý?ý%.»TTk?ë˜> N¿¿íA+®Ús~¿árߪJ¿æž©/"¿ÂúŒ¤¿ÙƒöduË^AGNbllTXS 1221+229?î[	'%?´˜Nsê¢?Y°@ÿ5?Y˜N×-Ã?©>¡(î²?´Š"‰
W?îmT7Ý?²õÉ­-?÷åá82?¥íF$]Ÿœ?¡0áG£Å§?ª}iAŸù?î)=ìÓ0?›—Ûƒ'Õ?fV'ý¾'è?b•U€Oǚ?¬¾°j?›vÐN´'?ì<íKaA?©;2—=/?‰\©GcK?|â?ñg£?ºüuÅä?©ÃªeÝ?íy©W/o?¸!â•cZ?p¤F™YŽ?m<èÔ@dÄ?³,æH£ü­?·üޒô?ì<Iã+'‡?ÃhZðš?¡R7XC?µH÷\ñ²?µ"‡Ëù®¦?¼ò¢¹ÑB?í	/n'"š?¢)ÈE ?p8â}ð½?ln†îã¢M?¶²öb_€?¢Mæu'èÐ?⼂k™oí?¾
Çf'ôˆ?¦Š©Z2Ð?£‰ìÕ
Eð?×µ¸ójà
?À.ѬíAGN4FGL J1224.4+2436?»­ÐS¹@TÛÀ~à°¯À8ûDæ¹ÝÝÀ;æàyQûu@А'‰Úà?ýג"¬Ó2?¨³×]tzP?©²Ð]Œ3f@ç|¯Ý©@¾wä"?ª¡;¾5ôó?±qÚbâx[¿Þw†®‹¿ÜKêd7b¿ãŸ¥'(^¿ÐjiÀ¸íGAGNbll3FGL J1224.5+2436MS 1221.8+2452?ïù¶*Q•Ò?5ÁŠU
?Tù-]CC?žŸPd:?Eœ·'ò1-?3¬Å2á?ïÚúFÇ?qƖٟ
å?@‡EãÀû?Iz£œŒgI?pìÝ6}q?p³¢Ã/³?ï©u;¸µ5?|Α^˜ï?^8&5¬‡?jòR‡}2"?Û­÷Û?x²Õ*ði?ïèEُ9?H¨‰)·½?B¾±'ÍÓ?)("ݘþ
?c@
ÐçÓR?Fn"ùŸþ?ïö›µ(‡?DTž‡Ÿ$K?$qKóÏ?d!>ßË?P:r '‹ü?Cø%…?ï•CI¼ó¢?‰·Žáª‹?Rh5¸€³?bßH_‰?ˆb+±C5]?ˆ]/Ýý'?ï†>†V#?€Lí§äd1?_ô*_~-–?cD:d¦Wù?ŠqÙ&Æj?~aë¾8º#?ïÉ.WßÃ}?cÜu…ö?UÉD±Ò¢?D¹Ž¬£Ö7?v#áÜ~pž?ar…8M¡6AGN4FGL J1224.7-8313?ì
•k9×À4e¿œb¡¶À9lʍWkøÀ;ü¢¥±ÕÑ@®¶â)Ö@Ø©_	zÓ?²¦_¿r
"?³¾õsµ'?ývqüœž1@
!+˜	K®?§]	pl#À¿æjW®Î¿çèGçöÿ¿éILÌKž¿åÓ´EíJ¿ïÿË&Ú_]AGNbcu3FGL J1224.6-8312PKS 1221-82?ïõÎîåüI?[£é¼5<°?*^O¢ã/V?,šœ Lº?QWÖcÍý?XZ<§E<Â?ïÖ®T‰­?t} Æç?Gšì"ä©C?P´·‡·3#?qµxSƒ?r#ûIšMS?盧‰!?xäÄ8÷;å?_I®ÛÜEw?e–ýïÄÈk?'êô¿	?v)qKóL¬?ï'M5Ï?c?Fró@?qðŸèi?Q­ªŠ½½?ƒ(º2e2Ø?]ø&Usá¹?ïæiôîÝv?c໐ëa?:ÿ…õîƒ?2â'|f?f6!N+J?bg^qñþ?ïÝùÎk;?Ÿ§VI?dU¬ŠX"G?rId&3,?Šób—ú³?‹Xô]Ánx?ï[ª¨,%ð?†ýÝO¡´ã?gâãOö+?iWG^i9ü?'˜Ž˜
ò??…ˆaºpf?îÕxoé?"‰G Óö?‹.×Læ4?sj
8ßa?™Æ¹–wÌ?}ߟˆ'ªAGN4FGL J1224.9+2122¿ênÍEn@TjWÑx-8À6Y‹zՉÀ:üÎqèz¨@ã™%ÖS^@9{úLaØ?'<cï¤Ï>?§|€Úš@aS¢>ƒÉ@#؅c¬¢¶¿Ð[¬Cjbõ¿â{R¼ev|¿å¤«{Cm=¿å³@ߙ-¿çÒ(@æпäâÀ‰Èk>AGNFSRQ3FGL J1224.9+21224C +21.35?ïà€¼å	k?bŒ™¯ª¯A?C¢BÈKe?<Ã_øó›?j–²iã3B?a[²8°v?ï›Èßò^?'™"GŽ92?[i¼‰ï¹?ivß:!¶Ì?… c!þÒ?'<ª¢¢Ï?ïYL2Ä´Œ?'¹:'3Å?p7Ï]I~ó?}Éêø
ƒ?È…ÈßàÙ?ÕîTIô?ïþɜk°þ?Pãn‡>ú¼×'TŸ>òÚÂN@QÔ? ŸÈ†B?¶G&Þ0â?ï¬Æy˜ê•?…QVbKõX?D½†þ>?BÄ ýåÂ<?ƒ'‰3z=Ï?"öE?ï6˜€Ñw? ]«Îw?m%`φb?…]{u)y?•ˆL#Ëà^?†NŠ½ãÅ?ï5Kͯå?"ö°ñe6?qí!œR?¬õžZ—?"ÛS÷n¤?"ÐÕi*Ea?ïýKº`?0Ân{½ùf?€="YÝë?¹C?1Ò${¿?-àþÅÍ(AGN4FGL J1224.9+4334?àzµÊ	h@R-gôÛߏÀ9çÁŸr ¯À<•ª¨µ–O@zýÕÙ:ï@kh¢×0?±ãˆP m?–œÇ nM?âF$!Gxe@ÁçAî
¿Ò1žBuÆ¿ä,4 ˜ü¼¿æ§‡-†K¿âÚ|îh(¿ë1Ûz¹×¿ïÿúŒ—ÓAGNbll3FGL J1224.6+4332B3 1222+438?ï›C_G°?}Á£°•$è?qS€e?eŽ<ÚØÿb?€n~«9Æ?v}í	cò?ïIò"­æ?§a²+ô–?ƒëeÎ?Ûd?——s¼Ÿ´å?•AÛ='ƒ? Î:…!Í?î/4ÿn¾?œ >_Z«?™}A	º²Ò?"c3>w"?¢l,¡³?'eäÄôZ?ï#ÒÇÚìí?€–
\¯º`?"Oô›.*q?|ú^¹òž?|Öɸ^Ãg?`w}†YÉ?îèBŸ•d´?"A 'm¸R?ˆ "
,q?bÇU؏O?–§bÝøó?òˆ÷t'?í»zpù+>?²äm§9'?'
.Ë%P?¢=Æ7›ór?«ÁÁ';no?«±¢÷QµÉ?ì÷ãr;íÓ?¢Ô'-?¢I™?—çé8dp?®9–¼²?š$HÒ?ížÌ(."µ?ZÈ"™#?­G5C¿?š[±~Í?'
ìŠ~ßß?|"çV"åAGN4FGL J1225.0+0330¿âüj´©ÀX@PcJ¡!À:Fþ»\bÀ;º2ƒàʱ@{õ&]6è@-{~%ŸÍ?Å>éõ§Œv?Ö,Ôz¿d@Q)`Kš2@×ͧS¿ÒÏß[š°p¿àìJ«õ¼°¿ßªT|ÙðL¿ê eêV ¿ë68Ág"ã¿ïûµ¸´AGNfsrq4C +03.23?ïLB¯Ž3Æ?Žûœ
ÅÓ?mìg¥¶Gw?f¦e€Ê'?'º~-H?0×Ön¡?ïØþ®òf?sҌ÷ï4?G©åXí&"?XüÙ–º?p‹kôéÎ?p>
r¹Ì»?êgÛ7	`?ªxÙ¹!ý´?©¤ÞíÇÕR?œ1H¨Õ?¿î¶ÎÖØ?¦Î»Q‰¼U?ï£ ùAA`?j´ZÚP÷Ê?IhW)ñJ?3Ä O¥/?…¡<N…Œ+?iØ#Ö<ñ?ïÚ¨qg?—)uŽ/TÃ?tŘ&Ý!t?l,MKÇXŒ?™3Dç?Þ ?•ÇŠÌ)íB?ïŒyÚÙÍ?œ\›õ/?Xsb½­R?höýh¸\?‰ö³Ûq?ba§˜hu?é·Æ3I?­¹øӞŸ©?®óC¯?œMÃó®d·?Äs^«uÓÛ?©ßø•ÖÖ?î¼²P¨A±?{GÕôÂ?frð¢¾Ö?WÈå3Ž^e?¢Í«î%¥?`´åiAGN4FGL J1225.3-3446¿'Éßίj"@;Èä†&öÀ;;ª]6;üÀ<›ÅPä@ e;Ó÷Ž@òü¬Žhä?¸xƒÚ¿¬-£ <G?ìnƒÖ¹µ™?þ¨XÓÖ¬¿áo0«¼²¿åT[זT¿éjêŸpž#¿Öö†oj¿ÒfuÞÝq¿Ý""ܯAGNbcu3FGL J1225.4-34481RXS J122534.0-344737?îԒ¬›n?¿õŐ(½Ë?YÊÅÒWß?U{»¹Ÿ¶?¡éæêÙræ?¿ýåQ0§Æ?ïˆZ\öXÀ?Œa± Ìi?efÁÊúˆ?iÌâõé‰?ˆ¸^ª?‡­Êg½Š'?ïF׿¼en?ƒÆܱeúñ?ckF*è?Xâßu&`Ò?"Áښ.®®?ƒ>ic2ñ?ïAÙ>óä?x!íh?`FüÏ~U?J­=è,$W?•»ý]ž¡?wó^'û©?îýË
¼à?–ŒPû"?k	cô´ò?dp^ȜkM?œår*×Ôo?•;¯&ËP3?î×zHÜ? P¥@ä:?u"*)æ?ƒ¥:Ëy®Ì?ŸÕðo»»?›WÿÍ(‡÷?îµÞ*7?é(é|\§?jÎÿؖó5?d¦Ù;ª?¢õ'î]Jœ?™ÖWI?í)ތNÄ?™NßàE'–?}4óŠÐK?rצ$®il?´à¨M-ޟ?™	D4RçAGN4FGL J1225.4-1550?·ÿïˆëIÛ@GHf^ê–À;Á_0ϬÀ<ÔL~]Óñ@"8u¹•?óv ž9%?æT~!nÑ?á–
˜à66?ÿw¤as¸_@—|Hzî¿î¹6b<¶?íkawê?ΞŠŒ‹i?íêó((Š¿Ä õÙ`ƒù¿æåfâOAGNbcu1RXS J122525.2-155251?劉*38?¬_/Óf˺?s¨®0—?¬r~À­ã0?x"w¢J+–?qc-ïüã?ïÙuV?wXI]'3?GâymÅ)A?f=£Çu?p€®¹ÿj?piN©U@?îÖ¯fà^Ð?'-)°‡Ú›?nà4RSõ?q¸xP? ³{‹õ=Æ?'pñ¥a]o?ïžÀkPÂ!?w¸m'HRW?>s÷?5-üh?‡\I!ʳ?w–üBEž¿?ïx2†Œ.?"®Á9"Î?{n:%VÚå?int ?"<Aw`3?'_ð;ìì?ï‡iYžq?3è=UEä?`–Â?þ?)ù‰ò%?ŠeÌ`áÚ?†è)AÇ?—ˆ?˜í5:.?n?ºÍT?o¢'a R?¬pSVíŒ0?˜ZnðÕhó?ï*íÕc§Î?"	ÉϹ´?E"êÐ<"æ?VÎ2Â8ä?™õþ¹?"Ë7e5ÔAGN4FGL J1225.5-2851?åðæÅFp¨@@Õc¡ À:……žÙÀ<\>ª_º{@¾DVñÿ6@¢ÃÉîËû?ÎRÚ'C?ÕX"Ì@Ž-À,«Z@	OS;;jd?ï¨3PD¼¿ÚYÞb÷F¿âQ žÛøº¿ì˜Á‹¦¿ÙàÀI±¥¿ïüvÄ AGNbcuAT20G J122515-284956?ïg	èØ®?‹du«æÌ?dÓ«.[£æ?^?ï®Ìû'?"M"ùÅÖ?‰3^›Æä?ï¶oúӊ?{? ;ê©?Z¼Ö|"a;?a,&sºw?~ÌÖ6Ø?u'dÕÓ?î¾{¼Ë8?"h¤aÒ5 ?"™8҂¹ñ?ƒæwEG?ãìÍ8
?'"@}ïP"?ïjtZšÖ0?l—ù¸;è?k¯2ÆóbA?QÝcQ—Ïû?Žwš™?iˆÐcz6Ê?îö ¡(aÒ?–û®ï)?si°›w˜?m¦²W«0?œQ‡µ€$ß?•Jr¿q?ï5§s:Îø?"T.Ïx-?oh1<Bw?wãÝçO¥?•^r%Á™?G8Röª¾?íà5…{ˆ?›ã
s3'ú?Ž2ÐP©ªx?‰$Øè¿®?ªoó•Ôâ?—÷¡0¨?îLâӎ Ù?‰üÙ7œ×ð?€üËñÇ4?o¸ÊU[ù'?§-""ÉŠž?ˆ¶^Ÿ"FAGN4FGL J1225.6-7313?ëHÅçÀ$é³ÃçÀ:0þæ$À<&A
çI@jђ"Q‰@0;7äs?½ÊÔÏû€i?§:{Ñ݂Ó?ïô&­é³@	JÊ©†ø?ïý•ø$il¿ÅÊEÞÜnÖ¿èÒ»YS¿×ª½®KØF¿äç¼Àæ¿ÜÞùÀJÞKAGNbcu3FGL J1225.7-7314PMN J1225-7313?ïBÊLa?‡ŒJ
AÑ?Hòü–ʵ?Ešh4;'Í?Š«ÿˆòé}?†Ÿ{õÙ?îh";¥Œ?¬Ã'L´‡³?S×=r^Â?d<	^a(÷?¨à<Î	X?«ú"ƒ5ù?ï? 0ð?ŠU&'Óì?dRR´3?bsÏb*Ðå?•‹×±y¬Œ?ˆÿPPÒ	à?ïrÂ$U?gGáZ–V?fÈõeýë?Eu'íÉ7?< Ì1?f#|*ÁÊ?ïGâÎýæ?'ü'Ç)C?Uû2Êù}?Ròk ñ n?•¿«•ß>®?'@J'×Tü?ì—Z\k?¼'2)mÃ?_Ê6Fšb?pъlm ?ºÈ½ôlÎà?¼/)'S?îFº\æú?›Ã•óE'??s=›¥» Š?q^Íø¿B?©,¦Ç†T?š¡ )H×=?îaãf[˜?ƒ;bë&f?¶'oá´m?h»ìØÃiŽ?¥t?¾˜ë?' XÆçÅAGN4FGL J1226.0+5622¿Ô²1°Òj@N4oÞµ,À;ªß<;À<ÉLÙÍfP@ÿñº—ëï@k¯–[ ¸?Åta¼2 ¼?iDúIÚ@JæýÐ?îÐó7š¡¿èá
¡~¿åáOp€›œ¿ãâ*⬲ü¿äÁt‹Z¿ïÑqÛÖUAGNbllSDSS J122602.81+562254.6?ïîRf‡Ñú?RɅ´¦5—?;ëm‡ƒÓx?+~úXi_?\`WwðÛU?Q­
{P÷?ïÌU"òi?tKêãnë?Hqw$›^?SÂËÍ~Ï?vÇ?"—­?qD+/±?ïo(Ïð?€þDn1?]p\}g0|?PŠŸCB??Cù…æª?€'VÐ)w??ïÚ Ø?Mçӝ?WY?ªA‰ò?=)Õ®?i³H,Ä£?IâÂ.1?ïÚVzWi?o¼Ÿu¬?I!¥°‡?>™ûÔ¦?oaBdÒ[8?mkj§ëû?ï\«ã¯Mœ?'vC…<ò?Y[-åßà?e/^7Nèõ?'ÔЬtJ|?O^
ܟn?îÓkaoS?ðâ°Ø³2?kjäeûÌ?e¥Œ°ÁÃ?¡›¢®!X?ŒÿÞléT›?ï†RÅI˦?px9\ÍøO?rqW
1†«?]JDîƒÃ?…2£!tó1?l.@Ñ«"AGN4FGL J1226.7+0637¿ïúXã4Üð@Q+OKD¢À:ƎyªæÉÀ<-†K<@!? &¼x?ùUɯáÚ?ÈG•*tÝ?Â[–ÿ‹eú?ý@|&©@Ç`QN|¿ïÿÿ&¦³?ïÿýç!é¿á3ÅP˜¿Ábº_aåM¿ÙVE'¿áYgŸ÷V¹AGNbll3FGL J1226.8+06381RXS J122645.2+063906?í Mï?Â
"þ1ɧ?c-•º÷?8£ûVÕ?±Q—'rŒo?ÁöxAÛ?ïÞM'G?pä¿¡,îE?@œoiɸ?JÖä9.yÐ?m‹¼Â¯ï?mëºî9ï?î47³±®õ?¡yèãԇ?x"‡y	÷?…ܹó¼R?©ªÙ3Š?Ÿgs¬ ?ï`j‰"F|?lÈÈs[HN?eÞ{·å—?JogIðÎÝ?'Q³c\À?kiQ«Uó?í˜ÀÒSۆ?ÁOäúk£?d:›þìä(?b–[²¿k¡?²˜$¶³ò?ÁGD¼a^"?ï'/r^lG?‡eZHìp?Sßk"žH?_š+œ/Zê?ˆø?ª*"?"ýð¸Áò?ízí'4èŒ?£ÃBP^G?w‰Àk!—?…B Åz —?²¯÷pЧÂ?¢"˜Ž+Ò?îeFÞq÷?‰6w	¦8?vO=ãC?d>S †+×?¦âÁªÕ-?ˆ1K°
QñAGN4FGL J1226.8-1329?´²}zÿÄ@Hxª*sÀ9‹}¼ÄÀ<¦†çæ.@LÒ*?þò]€
×?¸[ìÿŒ™?¾#әŎ@PŸ}i[@Š Õ¸"¿×y çÁÆ¿è7k§^¿ÈI?9%æo¿á€`"•¿ä¤&Eüd¿Ð7œ'"mAGNbll3FGL J1226.9-1329PMN J1226-1328?ï÷³_ŠÌo?S¼ö¶@F?*Áñ;È?%WÝvÄÞn?J'Hh¿?QÓtˆ
h?ïыLòƒ?sl•åþD?Kþʧfo?Sh
Yùr?sº€tÑà?o¸ƒœ†£¾?ïªôPÛuî?~ÿ¶,m?e#詀y.?uIaÜ] Y?óã]!4(?tðc6ÿn&?ïaiÞ&L¬?iç'ôÀ ·?eì"Âë?F@«Yö£?'?⁛?h"ª"p?ïò	ˆÑ¨?H6ÜÇ~÷²??4¨¬›¤Ã?5w	èd?TÃá¶ÿ´?Cb¸Ý*¸?ïe}lߞ®?'Íw^ߞ?^ÊH"ô?eÚ.™«ÿ?'c°¬ð3e?³	­'ë×?ïz˜íČ?í6oàj?e]ò#_Š?qˆ(Ræt?Œ'Ž5Q4?×:£È¨?îa¬«5x?‰£8IŠ?x7 KS¬K?_©¹BpƒÇ?¦ÞK®·àm?‡œ!/æÒ¦AGN4FGL J1227.1-4437¿ïð–PÂm×@2­}|,¡À;,‰ËÆ=À<šé+¨$w@!8 ¦n?üËyæuë?Ìc¶ˆ½©C?¶dt^Kº¿?흨;ic@ºì*
?Ÿ¿å­4¡Gbë?ï©3g#{¿êŒ5-w?Ö©aãŸÍ¿ãÈÊœ£¿¿r¬šÓ+AGNbllPKS 1224-443?ïâJìýÂ?iÉ
øbò?2Ž}lIwÁ?*'Œp¸¤?kcC†9'ê?g"÷?ïà얎Ô?tZ,Ê¢öÇ?9|£¯î?E·Eëë(?kã×fìæ£?r»'5þÜÃ?ïcw1Ç?ˆA^miR?V¶kUR.?VëÙ½t?'2jn/sæ?ˆÞjF)a?ïºãŽ/X2?e!€ ÔÂ?Pý1VKÖ?=ÌÂãö)?~Nøˀ3þ?c—ÉÇGu?ïÒÅô…<Y?o¤Ëc,«s?>núÆw
?7åÊ|%/?t¶$¡pS?n=3æu?ï™sõ×CZ?Šª¨-ݾ?UäÔø¦?e™=kTé?†ægí=õH?‡Ù¡ÏüŠ³?ïŒ?hö?Bg*GŽ?aݝ4ò¼?cuR(ø	ý?›Þ|aJSÓ?Œ²Ôàí#?ï8ã4ÜðJ?'•Œ,?io
̕É?bç"Î'›?•µ·¦W¿›?>Ñ¢^4AGN4FGL J1228.3+7521?æǧä,‡?@DØ	þ†ƒ<À;XèQ'NÀ<ý
)N­ã@<…—Y"†@è1AÁkp?ÑPÂœÇÌ?®Ùx_jÒ9?×w*#?P?ÿÀwÜÛb½?ïò…ÞѲ¿äʬ+l•U¿ÏõUҚl¿ås`'¿æ÷œ"/¥	¿¾[WáAGNbcuWN B1225.8+7537?ïċ©ÛŸè?iÀsªGð?D_ªj< ?2¯X_˜/D?{.5Ø2]?hÑý'!pØ?}Gî?ƒà!ÕF$É?buÁ	MC?e"ö‹HYF?‡ºýK،?€lG«U"Û?ï="õ•i?…aß·îÀÔ?k=–PöOñ?jn¾ïÕh?"箃Mî?ƒÆ·^LxÁ?ï˜h'B?dJԖn?n dϺtO?QŠõKÏìÒ?']ãð[Æp?`ÿ+ðˆ?ï‰}§Ë‹"?~VÅÈm_Þ?SO~;›ìÃ?LQ•¸szŸ?‹6¦ShI?}
û¶a&ê?îô%£+F?˜¾)ËõD7?jÍ"Zbj
?s3¾³?ž!»=bž÷?—§nJ^¿?î‰ú›£EP?'–NôJcR?wö¤Ñùäà?ulm5n¿?¤a§ÄÜg?B8]	^?îä7i›œ?ƒg;—À"?|-J‹Ëlÿ?iÿ¢Çɍg?œmÀ#¦`B?¾'üѵAGN4FGL J1228.7+4858?å;u 	@PíTK±¯:À9òÈlüÀ<PhÍK@áîÇôK@xéö©??»vapD?ÁA;ß,@ª#9Àëî@Þ<)Ñàˆ?ﲋ£6ÑM¿æ|zo1ç¿æÕ*Ÿû ¿ì%yÁâãå¿Ýì%!øxL¿ïÿjÿR[AGNfsrq3FGL J1228.7+4857TXS 1226+492?ïõ¬Ä2Ž6?Csf8®z?8#×
F<q?/'$£¥?M;WÄ:??Ãö+?ïßxü@,ì?l]°ñúu?A¹ØA­ê?K¨Ô!)û?lòœÂ$?gžZ7rÌÀ?ïª/ŠËå5?xl`‰Ù6U?c¯Ë8½Ö¤?o·NQñá?€ˆ*s€‡"?s14£qCð?ïàF™Â^_?M³
®!?UÁž¤Ì?>Èè@?dؗ(v¦Û?H$ ñxÅ?ïíS(#¾?TäåêºH?NŽ±Š	45?Ht*/{¦?V 
–¯Î?KT¬Im™?ï—?›1°b?†&ð| Ú8?VI{Mðû?`Ïz§$»?‡féÎMEý?"T¿—Q3?ïk©•Kgn?ƒnžÓô"?o7d¼áP÷?s¥¯*f7B?GÁr—e?7 ê7—?ïõ52?qàùW¬Ô?s´û(Ž—C?c3IN3?è54Êtô?m©·ÍJñÍAGN4FGL J1228.7-0318¿î¡âV²ûQ@Mˆã£¨çÀ:`*yPMöÀ<YÊ1çٙ@ê¢îþG@¦^ÛX?Á6šÜ9Ò4?±áàZHJò?ðþ ŸGX"@}Ðãe–¿ä¬ýpÇ?îÙE¶Ãv¿ãñ6É>£¿àTÞ긿åÏó'ªhõ¿íþë}'üAGNbcu3FGL J1228.4-0317NVSS J122900-031758?ïÌ;évaí?gÑ!¿èZ?P*CšŒÊ?9̇Ö%à"?u×z~?f''ÂNX?ïË4_
Û?wú%QŒg?R쌧	?ZÝBòk1?uª­YHò?rؒ΅Pæ?綠ÅÙú™?rQÎÖq¤#?Z-ó!ú?Tf"Щ
?ƒŠÐ4'¨O?pÒùÛk?ïKêmáHÊ?o'y;Œ:d?~ø'ÌC®Œ?_
?a:¶?‰¥«~Q?g^lê0'K?±~Ï?y&'ŒNž?`m-"ˆ™´?Q–†? ޑ?…!ú"ÇÏ?vöê'?ïm[¤&̄?ŽŠÏþ嶙?b5C]<¼?jڟµõÀ@?
ã
C?ŠdŸ/éNN?ïJª6†
,?ƒˆ•üÞ7Û?gŠwÂ=?a¢Õ¢&?"Çg桽³?êT…²îÀ?îPÏÖ~?‡8Þ°?'ÔYÅ){‹?xš®ñˆV›?¢ÕÀÖ
W?ÓB3½AGN4FGL J1229.0+0202?ãÊk)«@PwpyåŸÀ6ä^}cØíÀ;HŽyªæÉ@賖ðÇÔ@ë5ó×ӑ?Š Îc*À?¸µmŠœü{@"›y·|°@!¸j¢Ž5¿Ø®gÜÞï¿æ#
%󯐿éêPkR^¿ê‹*k
•¿ëó[ÂHf¿ëŠ
_ÕR­AGNFSRQ3FGL J1229.1+02023C 273?ïª>°o?Š´C‹gt%?t_DAü	]?†c"$7A?vcÎÇ?v—€Ì+"Ä?ïq¿$îvì?–ÐùšDÁ#?m7QHW?€œ¹-6…ª?ŒBVõVÅ?"15ÆÐ"\?íW	Èðc?§¥ŠÅi¢?§%Â"?¡Oɧ4?£iŸòG\j?ž¤˜hP¨7?ïùÐsþÝõ?7÷þå¹F?8"GäÙ?/éâÄíeÛ?8éÎX"Ö?*xG¯óbÓ?﷚BƒT«?€HþÄêç?kâŸr¥§­?kâS­ã8Û?vA ~}?zÌ̱Oìó?îÎhÿP‹;?©v§Ð+6?xž	´_^?‹'àæáÖ1? ®åa?¦GTj›5?ìî)[â?©:ô]4Ž}?©ÒZag§n?¢€6§I"?©òÃzhi?¡¡
"a.4?ïí¡ò6Fl?YSÝלï?S;
]øò?QÁÂ]Ø*R?QåÄ(-?Kkžb~{sAGN4FGL J1229.7-5304¿Ø0˜ŸÚ·'@#SA|¢À:lT¼ð·À<3uÇ,z@/äbÀ"…@úb>¹y3?·¥ÃH"™U?pN¦þYŒ?»breù7@	2tÔ¾2Ö¿Û¹4i"P¿Ø»b¿ã6쐷rÈ¿ãºI!²o¿Õ;à^d¿çú
­g¬¸AGNbll3FGL J1229.8-5305AT20G J122939-530332?îû£ÿ/?±d¢@ò?Så1@Á?TÝ@¾Þ5ú?ŸZ?Nÿ?°èRQk‹?ï;âm.<å?¡AP=–I¿?IpøjåÙ¢?\ß
Ü{?—¸*–fR? ­ZKh?îË¥Ú3|?'A{@*L?cº‡îP÷?aÛ݆
u?¢	ùÛ§Û?'{ËN'?ï´WxÅ9?[¾• 'f‡?Gä¿]Yqp?)Ó6rðW?kò%þ•'?[EKk:Äù?íáÕÅ;Uc?«bgp€?fCvça?[«=/´AF?°?9:"í?ª®ÀÌ}5z?íSª•?º¸ ÎtË7?_ëÖB?{í|qö'?´éšÿCnI?ºXœ—XQ?íšyÖ³3?S'ßž³?m–×?h4ÃÊNQ?²?†Ùœ•­?œñ4ʲÍ:?ï$ò]€
×?yá~ÒÇLU?a|> t?LéO^þrÞ?™>äÇ^[¨?y¡·\rÿAGN4FGL J1230.2+2517?îb/®•ô@U9ý6÷ãÒÀ8C-|:
À;pb·…<ë@Ë[HÐÿ7@ÝBeÖ?›±Ò vX?«Òƒšÿ 4@t/øì@ÓÐÜ{ì`¿Ì8¡1=®¿à‡ÂÀð¿áW_,¶Ap¿àãeË5óØ¿ä+4+€·K¿èjÜí¬@AGNbll3FGL J1230.3+2519ON 246?ïÔK^x0h?"gþØìÍ?Ežˆ—"?PðduÛ,l?s&'ŸÀö?'µ®Ù÷Ó?ïÓ؊ñ
?töÝ}°Ù?E¾F2»ý?PAû§È‡Ì?sÀÊß,â?sN.‰Ùõ?ïÅ@ˆÓ›?p=€Ç`ä?Y}'?ãz?e'ÆxÈÃ?wW/$ú?f´Fh¤+?ïü}}ju%?'/
VDpn?­01>ö
D̯$?9^pulŒ"?%⍝ÿ¢?ïÐíLæø?.¤ÐÓÆR?9êrà'^?:¶ÊGºC-?u겘'*?~>
ê"×ë?ï˜æ̅ݮ?‰èÙR)3#?RþÔÅ^U`?^{-/=?‡fr;5ÿú?‰/9g"~?ï¹á:?z''C¶B-?[©fA¿?e'[.?|µ¥DnÙ?wõ"ùp;¡?ïù7½Fr??\ÝD[Ž«?'dÕ+~Œ?a|ت›p?H|.ÞÞ,?>Á(qÀºAGN4FGL J1230.8+1223?ßMèKzÊ@RŸag#$ÈÀ8ÎIÚ>¥À;ân×N0@o&ëÒ Ÿ@5Ê¢P!?¤¾ÿô[K?¡íœƒ·b¶?ü84ú³@	=¿©"Ï¿Üj°¢õá¿Ø†3çüÔ¿ãBU&
±¿Þó·‡Á*¿æg;¾G"ÿ¿Ð6äΊAGNrdg3FGL J1230.9+1224M 87?ïâöbzüÿ?sFJX?H"½&릏?qU	¨V"?fènóN?\±M'yHj?ïnŸÌÓF¨?"½Èéü?lP¿n>ä?{׈Ž`2?CÜèg¡¿?'‰b¾ø?Ô`??'z€yÝ?_`µùQà?jÁSY??…t¾Û×Þw?'ñ¾x;?ï2×P¼ä€?vÇP¤Ñý?…·2Š*‹¦?jlPÊQG?'ù8Ýäo?l¿SÏ1…?ïÄ\`~?r¾è9Ö
?RrC"¬VT?HÞ5têÚG?y5>Ù4L?p'Ÿï?ݶvl?¨F}Âvº?w­"‰z¶¬?†|ºÉf§?¡Ÿ²ûNò?¥ê=D/å?ïjÁê=…?‡ìΕ'Ü"?ciœâ1?j·ø¥{Ï?E0ª¥'?†I%–p"?î,´@0i!?'°.>Sc/?™|&*ÜÙ}?…Rðy´©? v¨êú0?†'ŒÍìNAGN4FGL J1230.9+3711?íw*Ðw @SÃXdE#öÀ;kGï'Ú:À<¥}I׺g@:P$/µ$@"¿Z'È?Åáe¶K1¿³J²«¹VÎ?îÓë¤ÿ(j@‡/.kÎ/¿ÑÓ%•|)¿êµ
(¯G¿îÕâ Â?މº¾ØBw¿ïÿèÅPØ¿éièÑæAGNbllWISE J123124.08+371102.2?﫺mú"k?™Zè	èVÙ?`@³ƒ¸wN?fyPœ•g?7£ˆmf?˜l~Ï¥?ïÖO$7?z‡	XÔß?Eþ{_`§y?SáӉ~?r¬‰2[®?w{§q½?î)@ž´>?ŸÜvêÁJ%?tÕ¿WHÝ.?ye¶ó±ó?­R´Ý4ñ?ŸÈ'mú{Ô?ïÕÛ	·Ÿû?a"FŠÓ)?^"`fÂã²?T™ãÂê™?kÅé"K?ZÒE-¾?íãÀ&?œ™fž
ª_?m6`v"a?q?àÐÅÁÊ?ˆ
Á¾À‰a?™ôuåÈ7?ïOÎÍ-?ŸI¯Â7?g9$][;—?€WqTö?"5–7wV?›±Û>[ƒª?íV_hxíÛ?¡é±Yà¹?3'$ôŒÊ?'ï…{î?³&'–| ?¡ªÜf?ï@.¦±…?'D o«òR?‰ÃKùæ{ï?I'į¶«?†1
Y¸<¤?|–¶ãtaAGN4FGL J1231.5+1421?搸®ÿÿ¢@SÀY!À:YoÒòåÀ<]|Ìy1@ ©.§ˆD³?þ8RÆvq?¼é}1®ù¨¿vª­Nh?½Yۓ"@°ÊnΔÎ?ïڋ1!
<¿èŸݵR]¿ä7sŸ4
N¿Ó¢yg¿ár6é¡꿳ÆóDç›AGNbll3FGL J1231.8+1421GB6 J1231+1421?ïŒ<:h?µ'¨ìÙî°?Y§BHë?ƒÍÛsm¸?‰Æˆ©Ì–?²Ò" >,?ïÒ#K½ e?r*	¬µ&?F¦ðaWã?N¨¯"Ùh?t˜Œ¼,?p'›«)j?ïK3
!¼?…kÒà,èü?]0laV¡í?D#Yíƈƒ?"Æ—ûö
R?…MwâL¬O?ï\(*§°?oA×¾Õ×¥?o¥ôMɧH?QMm÷f?wœu•N?m'ëOCˆ	?ï'Z‡yË7?¹6|Åp?YKpÃÃØí?Mõ$֛Æ?ˆðƒ?€›¨"¶?ï^Ühîxf?˜lYBÝp?V!|z¯?^ó5%Øÿ?'Â[$€ø??—ç"tsŽP?îjk‰	?•Žh"0V±?hí_Öµœð?Yš/××Â?§ÊqswÖW?•Wæ×\j?î…"ä_!?‹Gº®ÜÉ?‡Wäj
¿û?pß9"ÖÑ/?¨±­¤¢è÷?Š³Ù4.óÃAGN4FGL J1231.6+6415?åÀ"šl[@J^j¹¦À:"k†`×±À<µ+úYÍÒ@ 0@ºÛ2Á?þƒ†'e n?·8Ô²ÊB.?)˜£i—ïY@sVOiu?ß^ќ•Lƒ¿Úª¶AÅó¿ã²¡r«ï¿Óù5@S­&¿ájQýù•ƒ¿ÄÁK#êÀÔAGNbll3FGL J1231.5+6414MS 1229.2+6430?ïâõ,+Eî?…xšIŸÄ?KDœ¶e$J?aëm–ÅJ–?f9¬Ÿ´Ôq?
>>˜ƒÒ?ïÏÃÿ–+?sáå#5N?H'Žêz?R«A¼yò?u;4õXD?pé{'>Sê?ïo»sÖ]è?ƒ}6»î£?eð˜D_?n҅{è?Ž"üüÀZy?€äœ¡‡¶Ú?ïšü½w¼œ?b5"cèp?p®C†OØ`?NxÍëÏð}?€é®ëG"¢?^{›3ú8?ïÌF0!A)?¡Ø7‰
(™?\'ZyâÞÌ?ƒqYà¬?r¸QCØ/¡?š*ÐÙ¹Ô©?ïU¢ácT0?›þ/i{Ï?[}v/?bœöòð_ê?""ÌiêCD?šlkȁâ¹?ï¬ùj1?ƒö-¶8?p¯h
\–M?rëxê?˜^†Ê¿>_?€þ»ÔüIÿ?î⥴…^?~Œè't1Ö?‡¿ '§Ð?l™
<>֝?˜iŸ`^?zÙöéÇR'AGN4FGL J1231.7+2847¿æ×1j0Jv@UUüã
®À8—|¼êºÀ;ÒÚý87@^ܯC?ÿFVüfŒ?¡šØÞÓàg?¤:à"BM
@	Dzãí@Û°ºG?ï÷ü@WÞä¿Þi"nå¿àWësÿߏÆ­°}¿à6YSXm¿åRÓº}AGNbll3FGL J1231.7+2847B2 1229+29?ïõ4ejñn?IL¢5»Ä?1pAÿãæÜ?'ÁTx:b?Q;$Þ¤˜(?Eƒ\Jùä?ïۓŽ£?n³¿™ë?A<°‰:>?HÉ°m?ä?p'c~4?k$G~	Š?ïŸ8"ß	T?€˜EÍs³?d,Pf-?qüÎ$??P?ƒ0Ð:…¡?z4uÚúñN?ïê4•š?J(þ•¤â?@îâþV9è?)Dð©–8Ž?a«ŒýXv?Gu\\ª'?ïñÒ<B?SGj—·bö?8"`h$æ?0m4 vÕk?VRïÔuJø?Q_hŸú?ï€ežÓ&?'ßÂÌ,Žµ?SªÁu…Ý?c÷·ž¿j?q`éšzú?'gÞ`ú|?ïbŽ<ï±?‡>'ˆ#2\?mÒ´"…ü?vïÇzÚW?çêÞ¦V%?"ˆâ@N?ïʲ9x?g\ܽ£?TÇ4áð†?GpJ#dn?uÄYÞí³?d{'0ûoAGN4FGL J1232.5+4821?íøzá®Â@Qm3	AÈÀ:%…—"¤À<†Ó«.í@Xûu·P@_ND0±?¸½gÔûox?³^óUw«³?ø¯²$ªÚ4@m™È"'?²PúŠet¿âÜb¡µÇοãø™]3¸¿çž<á²·ù¿ÜæÿŸ¿ïÿó v,­AGNfsrqGB 1230+486?s}é?=ø8¬^?ZB7R¸ù?I
¦Ø=H8?ˆR6ÕDº?€¡¤—±Ýg?ïĤ9bÖ?w¸m˜fX?Róː2?ZŠ¡êã³?xñ	l	Cn?sI÷Dðtó?ïX4uŽ³ž?~Ç­÷Ê$p?n£ÿ@?j±©'³4´?'$ñe®;¯?yÙhH·&?ïs[ö\#~?l³ fBx?·ˆ™P?d
ØëÉÿ?'K^^ÃL?c©3R+]´?ïY?{.ä?"Ž|Úñþ‹?oÆÐ3‰šH?f"'O±?™{þä&?"Õ¾Š€&?ïD*êdbU?'dw€åÐ?j<¦%ýkT?qùLate‹?"3
èXÀø?ÕFŸÊÖÀ?î'."'}?'Q<¼&•?'«SØÝ?zy$ª<}¬?£2;aa6?>¨ßñ?îcñÐx?Š"Mèµ?˜î/.R	?'ÖÜÀ"Àü?š"–»¼ÛÈ?Ë:ÂCêåAGN4FGL J1232.5-3720¿î<¥dþÝ@@9`ð¸,,À:'…€ÞÀ<M57ð1V@ Ӏñ5?þräùê<?·Óó?"ª—e.Ok?à3
^RÆ¡@ntÊ­7Ü?Òa¤W׿εœ¯x©¿àä/¿á,¿à)ᕱ¿ÉçΰқC¿å_iòâáAGNbcu3FGL J1232.5-3720NVSS J123235-372051?ïµlèzl?p8¶ÌÃ-?Sð¿¯Ó£É?BGW‹su?€<ŒÄè0?mâÆwå"?ïØy
Tt?q—uúÓ#?C´€¦'€?K™-µ‡‡?qœm–ý]?oÓ Æ˜"?ïtÆJG?z»Ò˜¯‰ÿ?]fŽTù?JOAªê"	?!­ÿ2¤?y؎p|ö?ïm1û5üø?g#K0˜_Æ?]>³O¾PS?@£opë†Ú?…Õg\!í?f@9Á@ÌT?ïiÕÊÞqK?Õ—rÈ?e{5m"š?VWÄՍÒ?5É?Þ=WË?ï'úçq—?"c·ÎxŸ?R.ËÚ[n!?\¦©?‰;lÇçPU?'ÕóܘF?îß#·SÊ?‰ü.£iŒ?kqñ¼Ð?g}Ò¹ß? [Ýr¹/?ˆ'ÁÄc¥J?îi:^J¹?…ÍhÙ&Z?ráßÛ&¿£?_ðm@N8?§ Ë~M?"Ymúme§AGN4FGL J1233.1+1703¿íN¾:Ò}«@SÄÝ?á—_À:ûÒvYùÀ< C~ÚÑr@ +ßâSG?öm9ôîT?Öç=¼N${?âX¼$@kªÃˆê@È]Rkˆ¿î™‹âvØ$?ïþT>p©
¿Ý¢¼'ý¡¿Ëvh›ŸÙ¿æä:ýöe¿ðAGNbllRX J1233.0+1701?ï̬«f˜?z¶ÊãƒÀ?dw¦è,?gɑœ³Ÿ?nÛ®IÑp¦?péÁDAo)?ï›ãbÕ&?ˆO¥?g¤,åÒ/u?rRø'(ªì?ƒU;Þ_ì¯?ã4nüÊÝ?îÜ¿¦žÎ?•Œ#Á#—?¥™(6&?'5)·[¢?œ~ǁ"Ë?";_[î?îý9I?‡ÏBÁó4S?"oýÂL»ü?}eƒ¹cH?¥Ø-ˆ½t?'àÀ5َ?ï¦QÔ;´•?…ÖÁ"
?u)£wFé?{›	@{‡>?w­r^€4·?u֛%âr?îÔ4
w'?¦}à˜£?''¥qÌš?Ö¤ÀRæ¹?œ8+¨jæÕ?›«?"0n
?îH²Ã®i?šÍ|Îqbz?"—S¸·W?†0*îÊÈ?¦Nþ×ì"™?—ív`eŽ?ìàØ¿Á™?ž8å
•?›,É@ñÐ?ì Vb?¸M÷Éi"Ã?š$_õwՓAGN4FGL J1233.6+5027¿Öâóç]@P›'ÿÀ:¼pøŸöÀ<¨~–ÞÔ6@€ïW¼)'@ÑyÚ·q?ÄÈñ¶f.?Ä·©º,?ýˆ¨°Ò@³§<ðK?ï¿ÜŽá¯³¿Ý#¶]ÞØ¿çJ¶!œÁ¿ç´Uý¸}
¿è,œ2¿ïÿÿ)@k*AGNbllTXS 1231+507?ïtNe,™U?­LànÅNŒ?}/ߘr?­1ï¢uò\?"Tw<«¹£?€z'lýx?ï
'£š?ñóØj?®5	-š}?x3V•8Ù?•RÏI˜"%?‹J!ú5Aª?ï?.
¡¼?‡'ù3ªsÔ?~¢"ž{G?yîôà@¯?•O'¿ƒÙ¬?'–'Ý›IC?îFºù)'?''å¸YŒß?Ÿ­ÓC{®6?~X
¦Äè?—'5]_®?vfT*ù¶?îŘ ج?¢1†$»Ì?‡ØÓ Žpë?'êË'•¢?›`',ݲ?—rÛîØ?íž,ÀIÝ?ª'öA¤à×?"89K]ô?•(äêi¯‹?¬ßaþ6?¤^'}p™?íú-†öT?˜ó§§ÛC?"0ÒØ?÷±?Vñ~\ý1?¦D½Š"·ë?'-ÑëÙ?ë'æyÇ?›üÆÛ3Qm?µ™ÀýRÿì?™:œ0R?±²'͔ìã?'qW1õXxAGN4FGL J1233.7-0144?·‹É#)bÀ@Nhj¹¦À9@'üí&	À<ð'Íó@ðGÙÞX:@a̾Šë?«'Ìx"n?‰ÇcEj\?ÝG¡Ÿw@
î /àÃO¿âù&Çë¿ä,ggfN¿àÊ1|yÎ"¿àî…ÿ³ÔÙ¿àÚßI§ÿ¿ß§†¡ð*JAGNbll3FGL J1233.7-0145NVSS J123341-014426?ïñRì>¶?O=àÞHõ@?5#µ¨‹?*ªÁÊÍÄ*?X7#Çt?J;ÀÛ×?ïÜÝ|%$?rßH>LÕ?@¹|žª|?N˜\ N?nô$ƒ˹?pžëRíS?ャºCïT?p~í}:Î?R"®ìp»?B
ñÑPz?|…}ÈJ¹?o¶Â+‹¢?ï½ÖóÓ]?^R½¤˜S?Yè ù¦Ê?=éf=‹o?zþ7E?ZHPN¢?ïݗבe²?d3yN
h?E"¦¥W¹É?7ÿP¹zð?m~Ÿ¿	Ø?b5 ÑI?ï‹+î#[?ˆO΃â÷Q?Uj"k6?aԙ*s?Š‡Ã–2Õí?…úAð¨X«?ïíq:³c?Š½-Q'¹?Xñ^¯gQ?Lcµzá&?ˆæwìì??~‡øá8?ï^4jã9?ymƒ?RäÉ?o¦f[©p?WÙÞý'½Ç?D¥ÛÎË?vF™YŽ*AGN4FGL J1234.0-5735?ámúXe
µ@É°$öYŽÀ9 ø«wèoÀ;¡Ç¯VšA@jª›6Ó?ý1úNX?³…	>Ã	U?Àú¤ÌR©@œZz@	…™0=4"¿ïùw»"€^?ïâY'kÍ®¿ÕpB½ê±º¿Ýa%^ß3'¿Þèê8v¿å=»ýœ£dAGNbcu3FGL J1233.9-5736AT20G J123407-573552?î?Q–—þÜ?°¯JÌP'?®ï׿Ë,?…w»jàÛ?¨žÐT?¬œÄ}e4?í'˜¼¾¦ˆ?·o(á›qþ?r?zÐfñb?}:Ù͜[?µŸBl_oi?¶ˆmrï?îËÞ׫ÿ?"2EÞÃÀ?x#O0+ü9?}`
,'Ø¡? =¨›ÙԌ?'{.=Ñ¦?톣éåȂ?†£Ö.VqÕ?‹O‹zêN_?f»Û', ?°`ï@*—¢?"\s;À"B?íڜS溒?±êÿæ•?0ÀÜ€¨?…Ž`óŽAG?®

%+®?¯Ý¡íaS?êMš?Ã?Áž]èW[ ?‡#uE¿a[?"-ö9V®?ÅW^°(k?Áõ'Sk?îî¤ûÍ? 6kn?'F8'ŸX?"ú¸º¾yÅ?«_‰ýj/'?œ8¤å'º‰?ëÉ[ÿW?žM¿üYØ9?™Ú:HÛ?€¸#¸åæÙ?ÀbßPæ€?*G_¿AGN4FGL J1234.7-0434?îü ÷©;Å@MWS£ìÀ:ó¥S?ÏÀ<}ÊÞ)@ 9훤`È@|ˆGä?²——`Ú¿Šu¨Î•Ï¶?ÈXŒÞö#@ϗ‰!S?àHLŸëÃ2¿×õp¥.£,¿ãæ~¤ ´¿åy0}¡@'¿Èüªµöœ¿ÞŽ{·AGNbcu3FGL J1234.7-0437NVSS J123444-043623?ïÂê×?lƞÅ!â?Hsåø*W?5t–>ÿ¬q?{æ'$
âä?k¨ÿ ,-w?ïа¨¢?oÑ?sk†.?C7W®]c?I9t³y?u‰<·èÐi?l²ÄîÃØ?ïxXG>Ù?wˆ"ãT¯¢?\śmí¸ç?U®ÀIcN?Žb¶ƒŠ8©?v°š\x)?ï¬?	flW?cª³2e?O¶i
<?8P—J4÷?ƒ=€©´ ?cwRoØ
ß?٣þU?{Â'V¬ò(?VK'îsø?GrM†Ìl?ˆä™á×»?z^¤7¬?ï†öDH?‡ƒör¢.Ë?QÐõ1r?c¤Jk–Îy?ŒP["?"öM°ª/Ó?îî¦É$n?‹Qbêàþ?gkCΗ–?eFŠUgfE?Ÿ=¾f'ˆL?‰Ò—UáLÐ?îáû½Ñm?"§ðÓ¸^?fóïf-:?[¸_Cè¦2? q)IJX?"™x¨'UAGN4FGL J1236.3+3858?Èúøaٗi@SoŽ`€sÀ:Ç{ÿTßUÀ<¶=Y&âÃ@íçÈ%É@`¡F6E?½Ša~†Sþ¿¥ ÿ‡?é؋Fð@/UÌ¿îîεY+?ÑW:Ä¢ú¿âé³ÊG¿ÞâʚÃeE¿Ûä×E Æt¿Ð5ÂY¬CÀAGNbll3FGL J1236.6+3901RX J1236.4+3859?ïèÁ?Ùgn?QØí™*pÝ?C ŸˆuË?1XÎQtûI?bv˜"'û?O/ñ–¶™û?ïà͸ã"m?mÞ³i}Þ??Ïî"S3h?Gæß ØS?k8IÊKü?i¥7å¦Ò?𢡄,šÔ?gõÐH¤«é?WÄÓ¯?\{A`è¹?';|ˆ´Àw?bP#iË¥w?ïÍXvÊÈÍ?TƂ2°8?YåB)½3?>Øö‰–Q?rÚt{ É?S¤]+üö?ïØl<¶Œ?av·âšíi?Pe.{¼
?C^£‡"I?oa,rQ9¯?^9"¤…[û?ïœåINO?‡Q4«!d%?OŽG¡¨æ?YÀ L?†ÍÉ'úæ~?…¦¦øì?ïi³e¦*ª?z낳6ÃG?`Ø»!%?a'Í®"ò?®{í¥ú?xÇ^ù]˜?ïfƒô…'??td•ˆÂK´?r7ñòjÒò?^~9ҘÃx?C	à–'°?s'äƒ(½.AGN4FGL J1236.9-7232?ï¦i‹´ÕÀ#bÀh ÓÀ:~¸–ž=À< ÕÓËò@3òA{ul@Øâý¹÷?È=~æ»?ÂØgµ›Ø¹?ý‡†Œv›h?üy6ð'®?ïÿ–¹‰$¿ç=¾Q‰à¿çw!r–u¿â=n€¿çç]<9A¿ïÿQ÷GËAGNrdgPKS 1234-723?éšú½Jù£?ÆUÈbɒŸ?xì
=Uú÷?u¨<šI?ÈÌ´¡æLÙ?Æ.mtn3?åùŸÆ%á?ÄdŠ‰œï?'Ä-Uåt?''Þ‡®a\?Òà}¡Éò[?Äé7ðú?í
Z†¼Ñ?žþ+!hpÝ?"Lû)ƒ;q?}çð•?µ
eƙ²?lÓ°L?ê"7"ü~–?•¡£Z5÷ ?¨
ê¸ég?'_ÓÂ
Ú*?¿×Nyn?•UL'Ó?ãpה¸?Æ6°ß[p?ˆŠéÊÖÊÊ?')ú–†Ú?ÙÇÙv?Æ)ʔ8[¼?Û5èœXˆ$?ËÑÄ÷Hÿ×?£QŠ†21÷?ªÙ^‡s?á/ó	™Ô?ÌQÉæjþ?é*'›?«¯[çJ?œΩÈp/?"Pˆãѽ?ÇÖxl.?©çdDürþ?â²âÚnæ?§¦±}b—ª?½A²§Ý"? øÞE¤e?ÓIÏNSÂl?©Ž tÝ«MIXED4FGL J1237.0+3019¿îfµª'†>@U`‡~äâmÀ;Ú¶\GÿsÀ<ëCòž@#<Ï8ŒäT?Ѭû¡ ¢?ä9ÓÀÝ?ïÿÐß´0@Œ•¥RÝ?ùl@ûÉ?ïÙÓ`dĦ¿ï;üR?íÐÇÎ`Jÿïì%W¨]'?ïæÑÆ0ÑY¿à¥è'%1AGNbllRX J1237.0+3020?ëyÓòõš:?Ë&èG㪛?Œ©56ü? ÁJfVÛ?ÀXG)_Iç?Ê,][ò<?íˆXÎ4J?Áž2ŸS?™cP5k?±'ڄXZX?ªÈˉӝ?¹òLΏŅ?è el&ªö?¶rTöX_³?©Ž–bf?žL†#^?É⫪Î?µÇ¶\yÑÉ?äïcšP›?Â[ºnƒõ?]hÒ$Æ ?e¸Rß!kf?Ö·bµàU?ÂÖ»ãñW?ë-ÐÚðÉN?È
ƒ;´6(?—ƒÎæ‰_°?£¢ù*Õ?ÀXB·4µ?ƪú¡É`?êºAñÖ¶I?ÌBeô.C=?°'LD(e?ÂF$ò¨©'?¹«¤.ÚM?Ãxæ%ŽYõ?æ8}²'º?»8¾ôƒ0]?¦÷Û‡{=?œ¾["ü+?а	ž zÅ?»bšc÷:?Úä·òlï?ÉLɉmÉÔ?K5
ªÊWî?XMàŒí?â†ÖÄz÷K?ÉL&aóÕMIXED4FGL J1237.8+6256?ïÞf"Mn7@KåâGˆUÀ;¢Qó蚉À=
]Qï@!Ã1Ãq"?ÿ#¶¾mŽ?ÊZˆâ'0𿧓¡2OB?Ùxœÿ§€@A#ݪÀˆ¿ÞGAÝðá¿èðk¢æIv¿æñ?Þ<`Ù¿Ïøö¡]¿Ø´^a4Me¿ÝùÚ·qõAGNbll3FGL J1237.9+62581H 1241+626?ïæ¯z½œ"?y®˜;ÆÉ?/jÔ~žè?*¼J6jý?gYØþT?y`BðžmÔ?ïÝÂ
Ò?n¬[Úó‰V?:?ù¶_Å?D'öƒ<?nõí­Å?l­¢­ñî?ï'Ƅ£;?'JYè?b(cîÒ?sw­˜`?˜Â#I€?''SúÇë?ïé&õ5]?Q°$;nÏ?5N8U û? Y'°Kûå?d/CXÕA?Q§z+äæ?ïÅã›_0V?{Â*39¦/?>®À½œ€(?;É0âSMV?{#F[¥{?zå©U
Û?ït› ¾w±?¥É:'5|?NMbžêž?Yiøą×?z3PNù?¤ú8ƒÈ?î`©Xý?˜íü¥áC?jGB¶hD?y=BiP¸j?¨Sé£Q'3?˜*ÃÆz?麗‰>ä?s"Ic@U&?QS"ã›Ø?E•c{Šá?"3k ×¥?s›nsØAGN4FGL J1238.1-4541?Ýÿ9‰Â¿@1df±æÀ:¡•ç]rÀ<MI)>¾@â
?#@*k
•?¹ÞÂÿª«Ì?µ b‹l?ùú>¥W<þ@"Ô§äá¿íÝ.^¸<?Êk|»<'¿ã€.Ä8©•¿âÆ®¥šXÜ¿à߸aÛ½+¿ïþE`zîAGNbll3FGL J1238.3-4543PMN J1238-4541?ïó£U&šk?Cd4½ÒBx?4¶–÷,Ë5?#öL;s@?S‹°3M^?@e•M¶C?ïݶ¾\`m?rò5…©'Ø?EAÿÒI?Q9ûÃE¤?mq"	ê<?o\vwÒ[Ä?ïÂ.6°Q}?k"ùø8©?XV'Ôº?_VísQ?xè¿'Ø?e]Ѹgc?ï¼	ÿïJ6?Vp#iì¡·?]ñè/ì¼2?;Åýëa'?z~…ß'ýæ?T{§"7?ïëö]6^X?Oœñ6¿Qá?B…¥vD{G?1åå?^ÐsC›?Ÿ?Jڂ³¦ì?ïŸéaØã?…Ô¦}0A?Zyisš*0?i~•cX?"¶ziÂU>?'¶­`~Ѐ?ï¡ÏH°¦"?s^æI³mÏ?_çÓ´(®M?\ø"×,܉?ƒ3XÕ7?pÁ­ÅW°ê?ïUÕë7#¶?tétYC?r'²þ>e?W®­-Dc·?»|f"£¦?s)0ÑGAGN4FGL J1238.3-1959¿î–'N£|@Eb´·,Q˜À9¨ÔÈCÑÀ<>÷ÂCÜÏ@BÙ¿¤p7@Ǟà*w£?³j·?-"´?­FæÄD½õ?øcì8¢Þ½@
JGB‰½Y¿½:ÙoÈdÞ¿à`ö…,û¿á݇?Nõ\¿á­%!ͅ.¿êöM½øô?¹ðCŸgAGNbll3FGL J1238.2-1958PMN J1238-1959?ïâÕ}©È?ZRí³Äâ?MZÁ"ÏÎ<?;¶Šë©ÐT?eÓѺ!˜d?Uø[²âw¥?ï̙~@ͦ?w¢gÐG h?Q¡Hè殬?]å-2¿x,?uJîR=®?rh‡LÀÅÿ?ïj\½p8w?ŽC'+/;~?YÅMpo?ˆñ¸ ,8?"U²…Â?Œýx?ï¶u[]#?[îêáb>?b†˜|5u ?DÉі®éÛ?{'þŋò?Wvèjf>?ïÇ&=]?p<¼s+M?a*ÚÉ£?UÉF‰ìóG?säªú>ð?hÍÑp©Âþ?ïfÁ:Ðéð?• BU:+?]²¢×H
?j•Ögg"ª?'L¸%±üx?"'T6õÛ?ïŽêq«ò?'²´/¸x"?…''‹Ë_@?ŠØëÚ?'úYeš?†ÐvÜrŠ¡?ï7ƒjê?à?|8Þ_®À?xö‰oÛ¨?cþ¼¹"XÂ?'Òý?v»u¥1GAGN4FGL J1238.5-1201¿ëÈÓ¥Gçd@I[ë[-M@À9{[ùûÚÀ<&=:óñÕ@	T¦ h@@휻	h?³c%ên?°oÁÙԝ&?õ1\#…@µòοT¿ØOãÖԎ¿äþ§°³'¿çõ²JÃÉ¿é2µßËW,¿îAy¢XZ	¿ïÿí )k3AGNfsrq3FGL J1239.1-1158TXS 1235-117?ïóѨ¥}?JyH[Ýx ?8Ì?G6?,÷Žê=+"?R) Pڛg?F>•
ÝÒ¾?ïÕåÿñä?r
WAi5?H~Ô쒬÷?TÑÀ}ç=
?qý%‡/~?m>‡=a5€?ï¹'Ñ!E?pɔ[[¹A?`¿AïB©W?e7ò?{Ð6{t?hgƤÈÙo?ïðT¯ëѱ?A;m©*é?Dl{'Èä?-Å)RV?U bÌ­?:ÑI(h?ïí£<c;A?UÈ÷©eÅ?@åf¼Ö$?3Fùûžøâ?\ª#ß?RЋ–÷%Ú?ïuÿ¹M?"ÍÈì?Vàg½z?e=öœ³6D?ŒÆ«OÃo}?"
•J·?ï~9¼íº6?}˝Nç8?gÊËŽËì?j'&ζà?Š~ÝúžK˜?yAÖò½À?ïӇš¤Â©?bPßUÙ?_+ôH¾j?PšcùŽž¬?lâkxÖ¡Ô?Z‡G}/:1AGN4FGL J1239.4+0728?ÙÏweÖã@@QˆÕ¥¹bÀ:;q¿_üÀÀ<lTdÏ@;݂|œ‰@èÿI Û?ÁfbàtõJ?¿˜á7èύ?öIãxà¼@%U-¥?ïù+
ÊÄ¿ÑÅJâÒG¶¿Ýò
ƒÌ'á¿æŠ=²èö¿çs[wN¿ÐÞÒn¥ÐAGNbll3FGL J1239.4+0727PKS 1236+077?ҜÎ?t‹š,Xyò?aBµ=?T98ñiF?…ÂŒX®S?rbÐé·?ïŸéô—?ž*¹ñ5?b ®\Ýn5?g'ÀA"?ƒµã‰ú*®?y1½˜ÎÑ?ïC嬆u?"H³›¬¦?p27w¥?o¯ùᏝÞ?"v¼Œóï?'PÀÑÝ©?îä¼ôxÉ|?x‰¬Qdœ?ñ…\Ùqa?pÅpŽ
Äl?"ož½R­ã?mÍ=Û¹ÁÜ?ï+
ŠW1j?†áQ2/y¬?x,¹âí?qCåÖ³©Y?"" w§}ô?'®ë'Eó?îû®Þ¿w?—Üì‰éhÞ?sáÓKs?x'k	 U¯?›'¯`|O?"÷ȧbÕÄ?îf1
zM4?"âŠ+ëZ?'¬>쵯?~poUKU?¤ñßj"_?—ÏwÉ{?í3PÊï?''øj©Në?¢{)8ðž?†¾ÐP^?ªS¼–n?‰.EŠ9."AGN4FGL J1239.5+0443?ïǚzVç@PÚôðØDÐÀ7†¸
"'rÀ;q'¬?Ž‹@àðfÚÕy@Ò¢§_U?—ê&yçL«?¿–ˆÌAâ@%|Q£"î@­ï"ã?Ð>ý'¿ázÌ_¶Á¿å%)œ±|¿æŠ ˆK>¿ì«»Û
p¿ðAGNfsrq3FGL J1239.5+0443MG1 J123931+0443?ï88ôa?'ŠoQ÷?€å<ª]:³?"S0A?†C*Á?ŠªüG­¡`?ï6Ìm+|†?dNrόb?~A"Àbq?RÃ'yÄý?'¢âÿÞ¬?"1eÓL ?쉨Yó2ß?¨¹ž_»¢9?¯ïp‰?¡Á^ÌÂz‰?§ÕŠòýé?¡ûW‡wïU?ïÐÕ¥ç?gæ3M!ØU?i3EŸjí ?`d¯¢•?f³å(òë*?Uí¿M²k?1X?š'0$Çí?"¿˜ÉEÝ?'Üc#0ñ?•n\´Hâì?–üϼ?îîû Ê»?°åmû?­¾?tlÁ±b?›7¹ñåß?¦Ãõ=ÓK÷?¬iõATþ?쁖ڑJZ?«rºsäQ?ª*I‡¬‰?¡n¦WÁR³?­¼t	ôä?¦n»A܄«?ï@®Š±8?ÉŒ³~°?~ºH¬:\Ò?uV¨Ÿ>Y?€R°g?uv©Qâé¡AGN4FGL J1240.1-6846?îjÓ§¦À²-"wú
À9à§7EÀ;çÇc×?í@ËÁPAáÍ@—Yûô؅?½Ñ¾¿?¶ÙþŸ¾ÝÝ?úCŠc›°Ë@ʯ‰ˆ¿à2Æü©3k¿Ý95@S­&¿æj]¡›Æ›¿âˆ?)5®¿äEœAi¬Â¿ïûC"¦%AGNbcuPKS 1236-684?íâ\ÝãB?Ÿ;ݽ3‡?t<Îuïõ?cj;«z^??¯JVg0ã?žHœJ$Ɯ?éÙº%Ö(k?¹ Y2h‹n?t2.³j"Ð?thïr‰l?Ç÷…ñN¿ß?¸•ŽtCì
?í0èeãe?œ~xæL£è?Žvl€Í>?'P\7.,ž?²¨ŽW[-?™nβ°¯?í…Þ¤«#?…ÅÆÊßu?\6Å`ˆ0?j™=ÔÐêý?¯tcàð³?ƒ¶ç1ûÄ=?ëE‡x|4ü?­$ª—3[ú?Œj0ûi{?{e¨§ÏÌ?Á#?!šž?¬!¬À?á­gèÙ?Æxãá¼H?Bjc™(?Šµ;Μ·…?ÝOÇQýgŽ?ÆrI¼•$È?è֍Di?­XXæûH?¡°ýot/'?Ñ=
Q±†?ÈY&pñÉu?ª¨rÙÊâ?é÷¸Í€@? ¥	dWÃ?¦Jwœ"Ê?ŠÆ-óč'?Ä)ƒ5mäÏ?‰Hv£AGN4FGL J1240.4-2606¿ÅkPG¸rÅ@BXc{ÐZ÷À:Ž£n.²À<;/•Y@€žBöŸ¯@¾¥<e?ÑFÆÞOâ?ÐÍž§ö?ûióžÈ­ƒ@¤­Q'Ñ?îê£aï^G¿æFGhÊ¿à×è‰ÁµB¿ßöÉàß(o¿ïÿùµc#¼¿ätü–¾óÆAGNbcuPMN J1240-2608?îÒÏ% +7?".Þ?™?Žìk< ?‡+ŠiÈ=?–/åì­'?†è¶-=í?îº3®"c¶?›3ӜtÀ?Œÿ™ÅÓ?Ž³‹Þ'?š¸Šb©tV?ªì9Ñ?íø6hO}I?›Â³ëG?˜á;׍P?'xíﵙ¥?¤û‰ÓÄ?'H´AQ?ìC}Ò­{=?‹¬)PUÂ? ¯€l¿x?|¸à4÷A4?µŒQ5~q]?†U0˜€U?ì«ÒçÕ"?¨£ŽØþçÛ?¤ð$8ñ˜?˜ãvŠài?°/wJý&?¢z¤Þ\œ?ìüÛlfŸ`?¬Zb;ÓM—?SÒ:
²?	ïðŸ<?°Ä0CBS?£ícÏZ}?ë‹ÔTß?¦ÐD~»Œ?¦ê£PK?˜i¶Û|q?¸,WNíå%?¡A½ÅW?ç^:Ç7rÄ?¡@²4¶?®Í»2"\?•no"j?ÊÓ¦–d?Ÿ¸IXøAGN4FGL J1240.4-7148?ì~/©Ìþ²À!ì´®ÈÕÇÀ9y=07FÀ<¤—ú])@ µß5°)?ýì
Š,>L?²'s°Pë*?—¥bzž¶?鍎]ü4™?ýÊâlFOE?ïö¯¿uÌ5?ì|c}ÓÀ\¿åÇ´_¾¿ÖÚ"zx—¿ÔŸ
â@ÒX¿äʤ~z|AGNbcu3FGL J1240.3-71492MASS J12402118-7148578?ç)fBv"~?¿z«Óê®? 
¥3y?{|…NÃck?Ñ0³PÖ¶?¿7â¸z
?ì':®*?¸å	Ï·Ë?s+?«‡ôÔ?€B8ìQ?½"{Gtå?¸7	ÎØ71?ì†HËî!þ?¢íœðÎû?‰°§jL+?…¤~DÁŠ€?¸«c‹3³?¡óØÞí?í.QÀ¾¡?'}ǐÏ?`D°«{f?²lώ)˜?®jÁ§Æ&A?‰€#·üAk?áTG¶´Û?ÅfZK"´?—&{(#?Œî«/H`û?ÜMþ*'Ш?Å_•bŽ{¿?ç\ —²Z?ÈKÔ¹D«?{3䜖àí?ƒÆüC'?ÐÚï?='—?Çô|ÖD?èþ¶3$¼ð?­ýâìºL?'Ÿ\g$X?‹J©Šr6?ÉÑ;§ ó?­"‹%ɤ?éýgKŸ×?¦o%!®˜³?°?ŠÓã¨?šé•'$y?¿Õ:ÑÚu#?¡BIk
AGN4FGL J1241.3+4236¿à…ÏƸqÝ@R˜Äq´xBÀ;²íþu¼À<¸M_.cÁ@ƒÔª;Ó@@Q8¢ý%?Åø\]#¹?Æ´¯Êˆ?Ï"jãù#?ü·»á2?Ó¤ —@¿ØÌÅ@'¿ê¸ÅCk›¿ïùϚ¦ã?ïÆìž#l¿ïÿþBe«+AGNbcuB3 1239+429?ïÍ<QmR?‡|ÞU"ãÖ?Yg§æ¯¾?vê!Oe­×?s›{¾Ì?|1MóT?ïö>Ž ?"™Ožƒ L?hl[%öÑ?xOí|
xT?‰gbf†Ú–?½«~<"?îJâ~ú?™3£Lt—?	À'ŠÎõ?Ž¦©–t¢?£[Å5ë?'Ò'ÎŽßP?ïæºÛCï)?W"&j§?-'~0Îrk?-WˆJ8??gküÌȆÉ?UíIW¬v*?ï©5ïXÆs?`Ä	0ŠŸ?d'%ö;'?k•lOÞ?€'ú¶ækº?€Ýë@ñ?ï+÷æ½?¯¾'Xö–?fšþЫV?}ò¤Â«'n?—¯Ï5DÌ?®Ã·ZŒÍà?ís1ãjF?ž1LãZF?—î'5Z/?"\]Пýý?¬ÕÎ7·Ð‡?—-TLJ–?"å‹Ç?}ûþHx+?UÊ7"¥g?\\F¶H€?ˆ('+¢?{§õ~ÿåAGN4FGL J1241.5+3439?ïÀ}wéµ@TŒ
Ã7!ÕÀ;'ë£Q©@À<¼tªÌÈ@ ŠõíØ?ÿ5۞÷§l?Äöš;*""¿—»£К?Ԕy^»¢-@|Bÿ*Ø¿ï´4_®t?î©ýýÇA¿åwø_!·¿ÄæËümNb¿ç†´ð75 ¿¿•°ÖÍÏAGNbllRX J1241.6+3440?ï–¦Ae? 
W"2ôÁ?GßÌVãx?V:
t*³?‰Ù¬«°x?Ÿ[£BN~õ?ïß=µ·u?t;ÿXdîá?@oˆÃ«õþ?J½™ìÜu!?l¦hb?rŠ¦¬èƒõ?ïvªÁ+¦C?…¶H"A?SɄUÖ~??e 6ãÒ?Ü(£Ý÷?…·ëòµrF?ïÏX°›>?W‰ÃßzË?^™¤ü¾H?FLŽ`e§?pʌñQh?S×˃v—Œ?ï¹],½›?†ÿf}›?G'[ë§á{?M5ÈðÎ?€6?´Ä"?…½š®+Fâ?ï•ðqä?‹F‹:íM?QJÀw½¨?[íe•¦Zö?ˆZ‹š[*?Š(N| ]?ï'$²
?m®H3?\ìÒÎÞè¶?QËÂ*ÆHí?œ,N@'8?
Ï‹ÊØ?ï|H5"÷|?u|"™?sñCùxØ&?dÔ:RTí2?†õP©¯Ÿ?qZˆ£YaGAGN4FGL J1241.8-1456¿á	t۟"›@GïAcwžÀ:$ÝpˆÿÀ<D¨ª®•@ 2J*°°?û3	wx¢?Á#øÙÉà?Æpè géô@8Œ{£åM@då²ÌÆ?ïï›2öÍ¿åhrû?»"íe»þ¿Óc҂™Lî¿çÏ÷Å¶¿Å	ä˜ AGNbll3FGL J1241.6-1456RX J1241.8-1455?ï··Öä=?oD?ק¸i?a_t­B˜'?Riãˆwö˜?{tZŽÏ³?jŸ¸ð؋?ïVÜÐÐèe?ŽŠ¼×Ã=/?t½TöÁª?x"þ},?ê!\Ì'Ä?…†®‡Ї?ï;ÛÅ°pB?†Îãg3?pY×"?l¶jIÇ·¡?"|Ç5eð?…ƒDr¿â?íVëœú)Û?†@MNÇ¡/?'s¹¥Ö?rÃÚýëgg?°ë´Ó㕲?ƒ,½»ždw?ïrUůL3?'K iù8?uyÇbCÝÌ?jƒ8?U	?ˆ­ªé:P:?~>ŒÆ¸Ñ?î:<•˜¿:?«ÝSD]ò?ƒ•ÃŽœ"Ó?‹ÍXö¬¾?§vÅÀOL*?¨‡z¡öy2?î<¸ø&T?–L»_õ±?'¬梿?"âƒom?§‰jÃàm}?"áÁ¤Æ?é«ï¡Qã'?Ÿîçð7â¥?¡)Xtþ]'?ˆÄ'š
¨‡?Åë^TÁp?X4käÌëAGN4FGL J1241.9+0636?âû­3¨é@QV'è},|À;]Å~ú±âÀ<¹4@€@!#AúÌ9?ÖcÜþô_?âÞJ¹a¶?ïÿwTV™@KƧïž@'™Hæά¿îáóFí$¿à.ŠÂfA}¿ê8¨½ùË3?¬!
ä­š¿Ú'¾1(—¿ðAGNbll3FGL J1241.9+06391ES 1239+069?ï¢Þk¼M?O|j¸ÉH?s4"n˜?xжÅ.1é?{» ï$?sïpÏüM?ï–qý&?"ƒÂǧ?gÃ*¡'"8?€¹y™V?"r¶Xco?Š±Ã¬É"b?îY¬fa?Ë´jˆ?—@/7S'õ?"ú'½¢ý	?¢zM‰w?•Çc͘?î:Ò~!)?—Ø@$[Ÿ¦?b¯¬P$?e?PÍuݳ?«2Ó9hûn?—Šg&ɦ#?ïf#ô¸	'?ãkN÷l°?"Mè»‰¼?‡¿ñ"çŸ?')tÞóA¶?~óù+Žoã?áA›?¬M­\ïð?yºvN$I?ìº§? æòr5Ã?¨?NGN?íh5ƒš~Ç?¢l>Q%`?–X¼¡ßÍÖ?"b'‡¶Ê?®PIwûá¤?ŸÎúµ¤xV?ì¨K³²Ÿz?°™A]'?_dºãË	?j(ÏpÚÍZ?º@zz?°ŽY
éÇAGN4FGL J1242.4-2948?áˆv¬.ǔ@@'-VÀ:ˆ<Ž%ÈÀ<7Cÿ3Qf@ìGÅ•Ï@@OÁß?ÐUŸÚ%zä?Ë9{â#¡?÷	f±@±¨‡s&¿ÀŸRK–¬¿èX;•ØCù¿ëukò—a±¿ïü"J|ûÔ¿ïªH]¼ÉŸ?§c¨¾GhAGNfsrqPKS 1240-294?nò¯"?ƒ©åɤ?qñ¦€Ý¶?p>!@r?~»7äöÌ¿?~<v{xñ?îûžhý?š™¾™Ü?†*Xð¼S?ŠA8²ã'm?•w8Êgf?QÌ+â?íö-–¶$?› RÛÅ
?–'ÂwTQ?'j2¶§®?¥[Åcüó"?"1å×êõó?ï  ŠŠÄ%?x¸>½+?ƒ°x ¬¬Ÿ?g~›3†Œ?'²–>?q¡¯¤ˆ4?ïq	'Š´?—'áЧé7?‹1«bˆ¥?‹Ce2ôCë?‹óúÊG?Ñœ}???íñi(&?²‡‡]Ü?ýðz3ÊH?¥=zòªûî?¯ñ-Ïý÷?¤¬F"´õ?븕Vؘ¢?§$ÌZ:'?ªµC+>kL?Ÿ®uAø'V?´à³²ÀM?žjN´`GÓ?ígz_d?˜Ð³º–º"?š`x'öÿv?ˆ˜éÆ4¾?¬XÇgèZ?'T7@²BuAGN4FGL J1242.6+7635¿Þ6‰ë%Ó@DCÿÞr¿À<ºSM"îÀ=2ŠÙã5Å@"o»'!­Ð?ú%kå+hd?Љ
uZ ?­öœ)øæ?ၽí@?ýɸl«¿¤· YfÏ?çïMËdíÀ?Ñö?âÄý¿æÅ!²­<¿ÝÙôhI?ÒÅ0"åˆAGNbll1RXS J124231.4+763419?ï˜îð§â!?‡àâ»mü?CXEÝ?CYîtæT?ˆ'~I}?‡&ԅFß	?ïiížËÔø?‹ò1¥r:?kWGTf
?nE8¥­3?Ž®Æn½6¨?‡V|HÄF?îÔ¶õaO?'nGEÔ­?…5p
8?ˆÓ'šÄ'g?šÎiXSì ?ŠÖXe•?î÷e‡ÌÆ?ˆzŽfŠ£ˆ?rfz¤‰&M?a‰ˆv/Á?œ…TŸ0à²?ˆ7½w‡Ì?ïD"ì—©'?'e>qu{?Qá›x…d'?R<Æ?Îý?–Oh´Nš¦?>¯w®6?î¤'¾¤¯¼?¡VHŠ<Â?sÒÅz(Ã?~eAk6Ý?£C+d7*?ŸéÊëhqÃ?î2"	PÅ?˜wãú+xÖ?†.vûèw?ŠéŠÍÂÎÄ?§R_OD+–?"Õ-Â?ìÕ²;Ñè@?¤tÁE‰?Âs"²?zÁ¶ò܈,?·/=ê5,K?¤˜§¬+íoAGN4FGL J1242.9+7315¿Óïè
?ôã@Eí?)
»EÀ;.W˜mI¯À<ò],+6@ "q!€XU?ÿ¾ü)±ª? ªõ>¿£ð<àÓa^?às–V;@<¿á¬Ø¼?ïòÒO̲¿éÆ	>˜7¿ÐõDz®Fû¿ÖJªH=†s¿ä6¼ÿŸˆ¿Ï¥~ª*
–AGNbcuS5 1241+73?ïÙfDåœ?bXHV‰?E¿×Ú¾›:?4EŸôLh?p"ã
Vy?`՜Úr?1Îâ¯?"Øs¤0"?Z86Ë|]?[cpšù<V?""lȦ¦?'P¼Iá?ïms¯›?w"q"vÕÙ?b‡œa$Z?c'ÃvjË?©þSž?u
QR#q?ï{愝¢×?m=<ëP˜	?mzdO«Óõ?M™tÅNT?‰§ÅÐ[?mÇèÁ²Ù?ﶥ«?t‡ xQ¬?SÒUº'ã?D'—&؝ð?ÿáÄÐ÷?sG³äAµ6?ïÛ,‹ú?–QÞDˆ¸?d´Zç_{¸?mˆ?ñÿÔ?™ùy>ŠsD?"³~x—F?îÙã¡®µ?Œ¬»Ù Ë?f)%R.?_R㚡-ñ?¡CW#Ņ?‹þ	Ì*½"?î\4r½%ª?‰Yýé?"dÿ¢ñ=?l³q
f?¥#yl?‰—RšãŽAGN4FGL J1243.0+3950¿Ç+dÕ1>@SKGyBÀ:ÓG:Q5À<–jùs@ûrC>n@ÍÓB1Ó¸?¿‡î`ñ1†?s—'ÝR8?±böð6ß:@tà*?ë—­µ°¿æ´:æ…Û¿é=Ú rfO¿è:ÑÂÕÓ¿ð?ïÿþó…õAGNbcuSDSS J124318.91+395117.7?ïËåۀ]¢?mXí׉?uš½­ãd&?+Bñ8´I?QÉRJvÚ÷?Q†‡ëtj?ï†ñýš`?'¤ßµí=?ifaèa*£?€ãáS$Ý?‡éè N?…6 '?ï¿Ææ-?‰2i¹Ëöá?€ÝÓjØ´_?'ÀEsàI?•9lC:?ƒ1Óyµs?ïÄ0Rûqó?dßbUԀ?rx³æŽú?aèíãÊu?gÆ»tåw?MuôÑ@?TØ/¾?™^¤=F
?ˆŠõðe5í?˜öŒCù2?VG¦'?EÊ?V‹ºVu˜?îÀX'¾3,?¦íq8û•?{ô'ƒˆw<?Ʋ¸kÅ? {æ'	íÛ?¢1<ô35e?î?ÚAe·%?—möDî±?‰qÂÖwó?…Á'DRM?¥¥ë6šEç?"àd'÷z%?ïߣzT@?ˆ4ñ¤Gx?'íÊíñØ?ƒì¹µ™ƒ?…­×Žþ¨@?rÏ>ìú¿¤AGN4FGL J1243.2+3627?à¦h¿Î•@T œ^o÷àÀ8d çk´"À;w²Ý7~@¸Á¾Ñ·m?úa
 ë2?£k/MöX?®#ÃöÝ@àj¾º»R@oÑ^¬Þ›?ï>S¯­'¿Ô^ßY—K¿Ùß͚ýòµ¿Ñeœ\AŸ]¿Þ"Þð¿ÛWQ`ñAGNbll3FGL J1243.1+3627Ton 116?íìØøÌ|g?©ÖÛÑC÷H?xÑ1ïþñ?sÚ}èͯ?®J4¿/?©6,CÍ+º?î¿útƒh2?²e«C‡Œ?mÈÿdƒö?§ œšº]?˜IÌøw½ª?¡'4!Ce?ì;/µ
Ÿ|?¨Ò1££ú?'t6ˆ¨/´?'ÆÓP®ö?¹‰t·8Æ-?¦¯Ö"­?ëE'õ`iÍ?ŸXDS…Ó?¤P8È-á?†˜<"‰N?»«TWC"?ž	ÿkA#?ë›Z¥#Þ?³E v—0ë?Š0Ä$#ú?'ú¨¹Xaý?¿ßæË?²3SÖ¡å?íM^åé~^?¶æU~Ê{Þ?›gé­µÌ?©>'‹yà?­vÌEf²?­;.q…èÞ?è±áRڇ9?²÷-¯3ác?—Q™r#Ö@?'§[@pó?ÊNG‡dI?±Çü'Š0ç?çî×Ù<¿?°SÚ¡?°h«;$?šá^̋€Ê?ȘÅoqŽ?²,@þùAGN4FGL J1243.9-0218¿éðÓÎYü@NA	Ö¶[À:C(0 ±¼À<f/çCq@ðÒ]…l;@]°µ??Äv¹Å³þË?ǎ_ê o·@w¥ôïp@au¼o²j¿Ý<û ŸÈ¿çËÿÚ@S¿Ýæ"Cqò¿ß[é€Óô¿æצ
4¿ïós_s-AGNbcu3FGL J1243.9-0217PMN J1243-0218?ïëN»'€+?UÎS<ïpÐ?F98æ½m?<mšá.-?^Eì¯|k?Q:y›åå?ïݜÊãt?p€§šå$W?>‹ð`ëG?H~,îFoÃ?n'·³,Á?l¥Þj׫?ﲺVÊßY?rô`£'?[[ÏÇƃ(?W¼ž®bȲ?ËàšàB­?q2F=Ää#?ïÃpcÈÛ?WÙeïk…Ò?SÙoÛ×ð?3ƒk"t¾?y'‡JáÌu?VŽ@ï
C¹?ïÝú!Ôb?csÕ¯[b%?SGÒÕ+i?L "žL"?hbU€¸?^iõWQ•à?׎ò¢?†SÉ,Ž'C?S¼d
¨V?^?ÎGYY…?‡]Fԑ‡?"M?°èhP?ïoҏ?µ?˜AÜï†Â?k &@#Ž'?l¡zʲ§n?PAÍ/H?z›ÐÃ3ìK?ïX¢¶}?xz=†dÞ?gáv
öä…?Pç¶:¤?'ïF€[Ê?v²Ái/"(AGN4FGL J1244.2-4956?秊äiˆ@)Ҟ²N©À:‰XÀ<+©­
å@Ê	rðb~@öäÎ?¸¯¤@î?›C‹p*Ö?âª''¥@ÉbŠ
à¿Ì†9•w÷¿ãª3z€Ïž¿çŸÑâ5iÄ¿ßk*ñER¿äóý">5Æ¿á…\€‰}BAGNbcu3FGL J1244.3-4955SUMSS J124422-495422?ïÞÁ¼X?a0´Ä;…r?A	•	yí?3Mñȹ?mûÿ¨‰Ò?_áÄIQGè?ïÓ}
¥b®?y–ÜqKÅ?Bø¾§åæ?O:á&b?sâaYUâ?v$¥4|?ï"
§™²?y^ø‡àd|?^£ó‡p%?\·~صO¹?‡h¬Êó?wŸB5'å?ï«"'0®?Z€'+R;|?]æ4%™;)?;¯Ü5O_?É?XxŒ}*8ë?ï´ÙR0[?u¶lvvœ?SX'N)¨Î?I	p³.w?€^›/'(?t
¯?7?ïs ZËJ
?"(ùº±?Va¶¢·Ü?e²¿;Ùj?%Ù;AµÝ?'2?ʳ?ïÉ¿Ú©?ŠÞò™Y¸?l:"ýªŒ?dF™ d?˜Ÿw^n:ê?ˆ·©vœÄ?ﶏں1?yzdNûçö?vVwŠü|?ZþŠœ-?˜sL¤º?w3<'2j1AGN4FGL J1244.5+1616?ܛÄ-ä6B@SÂ=ÿ?àÀ:žÝõ<ôÀ<'è5Þß@l¦¿òÉ·@¨ _ñØ?»sLþ¶Så¿£1ÁKÂÕ?èIËÆ<Ó@€LÁz?í"ú¾z¿×9ƒ@;Ú¿áMÖ¸ª¿ãýR ^DY¿ÕïW¦°'¿åŒµ_ó°'AGNbll3FGL J1244.1+1615SDSS J124444.35+161621.7?禮OݸØ?xU{Œ¤"?`òU´Ò]?O|M6
·°?'֓6‰m?vNI…SM?ïµiȀô?…;9ü?Q¬bG–k?UϊZÏï?€p/û^ÈE?ÛG&ÁÒ?ïKq`'´?ƒŽ†ùÃ?lux9'?j™«{R?"$ú?´'?°\JvûC?ï;¬Øªjf?s]"žÿË?€|pðTO±?fOQÓ h?L,m5&l?pHôÐËÙ¹?ï?ÿ"Å6?ˆ@5cßÚc?t¾g|¹€"?e}.ïI«ó?'Ðs `³?†´'ëÅù?ïÃk¶B®?š¿Ì¡=Y?dD0S
?oBÄþ{¶O?š~ފî?˜Öµ{Cå?îÀ"÷?ŽzÂîñs?ufCÝK´W?lGW0T7æ?¡R֏äÒ?‹O•)?íªªÖ'Ù?_è,€Ó?—¤ô	µ]?…ÏáDÍI?©'Ø–g\œ?‰ïÆØß-6AGN4FGL J1245.1+5709?àx:¥Ý
¦@Mùˆ MÀ:>¢Œ‡b_À<¯è+Íä@‰€Ç»–@x\È_?»KË@ÁÍQ?¬ŠŸM/*?ñ××ârP@³£ùnìG?ïþÂ}¾qÀ¿Ø£k_I'™¿ãŽ.+ŒuÅ¿Ú~(Õ!°¿á©!âRðé¿ïÿâ¾÷!AGNbll3FGL J1244.8+57071RXS J124510.5+571020?ïëÖóõ¹3?Q¿$ƒC/??iò+¿š?1%ژÕ)+?`;Íò¢Ûs?O€çPnç?ïÙ7T°?r­Ìî»ù?FE‰'þb?Q0.Vë?p›ÅŸX3Á?oÉn}@[?•so8?x<´J!dz?XôDº?VùRç¨?ƒôRDh'?w3v‰{º?ïÀd%2X\?W«Ï}¼?lIäØ]¦?I¶Ë@ÕïÓ?q¨ûBO‡?R}îvJt?ïÕфÜ7?fØÕË©?Q1©Gmò?E×EQv=?pÊÓ<™^™?bêD%©{?ï'Å@«/³?ŠzûXWXL?ZGÖ5Û¹?bã)ä-{?Œµ
ÍÏÕ?‡¾x¢ÞNÆ?ïlÖ✺-?p™¬ú?bWšýç?`Ô*.ˆÇ?0OJd?€2KϲÀg?ïY,ââ
?tçT¾@h‹?'/b¨E Ê?gzôóÉo,?‡‹R'{þ?n¶–ëÄ}¬AGN4FGL J1245.8+0232¿Ù Ô¢j^Õ@PX4Á¨¬\À:ÒùXF3À<°·ŠEhÀ@‰Y"Eò¨@cIÙgåÂ?ÇҁÀá²?à©=EÛ¬d@U$¿ÒéG@-Äq3žé¿ïâ^¯c?ïEmþ
\z¿Ú!Ïþ°t§¿åÞ¯6'¿í8´FÄ	°¿ïýðƧÞAGNbllNVSS J124533+022825?å·d%"J?Âã#®äb?М‹ïëhw?Á½µÔì?¯¥^+«ë±?¢vð¡\¿?êf¶)6?ÁNDí«û­?½b‹Ùp&â?¼pMùeº£?®Ï…¶N5a?¥I:¤Ÿ9Ê?äîZm"±õ?´ð°,E<Ò?ЮƄ'?³4aÂÛ?µÕ
}Gý?¡{Q{ñº?éŠ)EüJ?Ÿ!<æBX?ÄnGóÖô:?L®½݈?¥¤Ká@Qs?ˆž)4ýnÈ?àw§Z«?Ä'ZˆÚ?ؖ8";Óã?Årú§B?¹éåP@# ?¬m{–iÝk?äÿ=¨µžæ?˟ÐZ(H?ÌŃdEqF?ÈkûdŠ>?¾{í|£G?³ª†«?àWîò¼?º¿/Ö1zv?Ø‹…žî?»I‹']E‰?½9³Þqîb?¥Ðèã?á/3lLJ?±ƒµŒ°?םjÁ%5?²^uË?¸ï-%Ñ?žù ‹|¶AGN4FGL J1246.3+0112¿" &ƒOêÊ@Pʽf'À;0íæ²QÀ<¦¦3
@ºþ‰³G–?ý*þE뜜?מքÜs3?ÎhìƒK?öz¬(©l@o…r›(¿æhŒEô¿æ¸Ã*Œœ¿ä÷'î\i¿Ä‹í¬vì¿åïw‡ R¿ïù}š_'7AGNbllPMN J1246+0113?ïïs˜~§?Pq9«ØÃt?9?Ôý	–?/¼Õ]^/ü?ZÉ»œ?K«u]Ý°?ïÖØí?p™B\ͳ?@í©ÑÌ>?IÖ¢9Õ?rØÞN?m…Kˆém?ïve!dê?'_…á?b¤¼0Ÿ‹?d"½,±dî?½ˆ¤8_ì?¤ 9m^?ï,œZ?f:jû²¥?X›º@c3Š?A¯ažéfÔ?ˆç½'Ƴ?e~Š½½I$?ïÛsùCo¹?ce¥Š\É?F¦…2V?:8ÄçgŸ´?oïMúæ?a‰¯v¼© ?×èߨ?ˆ&˜[†,?Sãþ+'Ä?\«ª‹­?ŒžWû[ÙÚ?†»
l+´?ï'/u—?%RÊÓ"|?i[
˜Ë¶?jNªr¡8?›XaûN"?Ž;¥mn_³?î͂¥óU^?†šw
¬5?eÎÅY•ºh?\‰Ê!¬b?¡ÊéH³–ÿ?…Ç13R¢AGN4FGL J1246.7-2548?ïþ¦b™—@B‡jƒ+™À7]M•µ‹À;>Ð}[ur@õ@Lz@¶ŸÜ©¹¢?"i†<«¾?¾îܗ8@'w,¶Ap
@ð‰JìãC¿Ê,jÈÌ¿àf¤^ïy ¿ä؅½™©	¿åÿdd-§¿çȽ¼
¸¿ï(	3…iAGNfsrq3FGL J1246.7-2547PKS 1244-255?ï'zã9ån?°Ú4	4¸?R÷ͼîÖµ?W¿'©D©?‰M}°[²?°Û~¾Op&?ïæRžð?ªi×!—×?ƒ>È#c'?¢šÊ
ïý?•cÙÌÃO?™ë|AB`?ï( öÎ0®?•]"rÍ®È?ç³áwz?'0Útrq ?†g2!?ŠG§ßW"æ?ï<7†Ý‡ä?ˆÿ5Ò5F¨?†ŽBŽÊýx?~3}êì9{?ŠcÛ¬™¶?yRù¯~gJ?ï¼ñ_Jµ¨?}ûȾ˜R,?W
7F×?˜?^Z#2š<?{Ä€°L?zÄÓTöü?ìätƒàtÊ?·ç¤ÅjÚt? AQ¤²‡?¨§4'€²Ê?°»³R…çi?²"½ûìO?ïËí´Á?˜Ìáó#?ŸŸÆn	?'«m<ƒ?ˆÍńÔNJ?ŽÆ}Î"g?í÷ÕTäì?ŸÁâuoŽ?›‹
î2Ö ?'µÏ(sq?¢½#Ét,ì?":õjüAGN4FGL J1247.0+4421?ïРjTmÒ@R0
ú/§À:j1ί%À<}ËÆ<Ó@ T¸?ú+Ì¢¢&?Ââg=Ñdz?ÂsLhckµ@óþº…¢l@šˆÙ-m¿í3e"¤7¿È[QIô•¿¿Ø¬@»1ý¿ÐÑÑCſܨݤ‹e#¿âüê×yÎùAGNbll3FGL J1247.0+4421RX J1246.9+4423?ïèXàR ð?a;·"6?A̔c­F?Ay£è0¥?ccl•ŽIë?[hrFü¹.?ïÖlèü·?t®síÎÕ/?HK9 ·>?Qª€}?qɧ'&<«?r+á]|?ï"eéÏù
?îyN"J8?UÒ¾I~¿?GÏÅøqKÇ?ˆl-ÆNèÍ?¼:OÔv?ï^õ®ÃL?gKj6Î9?g"àcä,?IÁÐJ—]?ŠC
r÷å?e*֊C?ïÝÛ77l?d× ÓY4Î?Q8Ìûèå?J{3CB?iˆbNþ˜?`/"gº?ï†ÎéæÒ?Š¬'8º?W»5ýf=d?b"¢-È(c?‹TÞºÇ!ù?‡ö=ÿ!?ï^^]ê}?ƒr'z­i?`´D"+*Ì?[Ÿ¢['Ý=?'«´À?'½̾}?îër×Zg?'îá"…î?wÿ6t¸??cÆ¸ßУ? ÅbS@…?º,nŠ°AGN4FGL J1248.3+5820¿×'æ{ì×Ò@McáÁP—ÈÀ7²ÂFbÀ;QDy¬"H@#'0iK?üù!ÚE[T?"ZýU­º?§]®1S@lë5m @²ŒI¥¿ºOOŸx+¿Ü[é B*G¿Ý­2=>ú½¿ÙŸÕ]jo¿áGßÝË¢«¿à;‹ÇHÿAGNbll3FGL J1248.2+5820PG 1246+586?ïñ
÷dzÿ?Iðï²N$?0÷{Ó¢N?"ÁƗ¯W?Y¦-{¹3é?GùûAä?ï|Ec"?pӘ<#&?hØ»Ïk»ú?ynæ"û{ˆ?Š¸x=9­‡?ˆ‡7èÓÓ?ï±å
g?€PܒÚp?aÁÉ= È?q""M¥ÏÜ?~•¨º$?|syûhÉ?ïXE ?wâu­ê©?mñ¼îwà>?S2O|wÇ?'1¨V'UT?vPš wû?ïæÅ7ñͧ?[·9ætI?0J‡]Ÿ"…?$ê,ÓO?g1wP¬[a?ZM=48Î?îÙÆĹǦ?¢ùÊË5‹?vŽt9<·?…‰´×à¨?Ÿ#Šeøl?¡>&;´ÿ)?ï´UšfH3?€÷4¶ÿú?cÐ.Nš‰X?sdŽO܇»?{톢%Ä?zKR(¶Ái?îÀŽ®3?ú&ý8Þ?z°-ÈпÒ?iÊ='âï? ¡bQ6‡?Ž‹¤e.ëÁAGN4FGL J1248.7+5127¿Á-BÔ÷ú´@Pj:ÀÆ.MÀ:çÓƼ"À<Ö35·qò@ýV"U@sˆ€l¡ê?ÀOBßN…?  ÜÄf¢?Ðσ@;ÚL@ô%ä–.?ïúKUhè!¿æӀ y\¸¿Ømû:ôG»¿áTBý«'ê¿ä¬œ«¿Ð7h!&–BAGNbll3FGL J1248.0+5130RX J1248.4+5128?ïō™ƒÛ?—=ŸI'+|?Jó~쀞?96¬Dl¸?yÚۗŽ§ ?—;·i¢Ö»?ï̒ôӕÙ?rŠ—›¯ß?H%íŸ0)?Qx(,ZV,?v±ÇË¡¢©?oœÉÂ[Ð¥?'92"?vß»LÖÍ?_uiߥÁ?Pïjם_?ŠïùÞ.È?uã¶w»˜[?ﵙX<hL?\ ßÃOn?ea˜Õ?E/€ãªe ?z§£8e?Y&@î÷?ﶞ "E‹?vú?,€Þ'?Zå¬Sˆ?LyH	Ðf,?~)v9ý\?v=iÆ®×Å?ïo"$¤=ü?¦Øڔ?V–¿ˆK?^/%í1?¬!ù¨a®?‹ŒÖ
Ù¬?ïÕZ?…"ðp¡B?hòçè¸Z?`a!=Ÿk=?œf÷â£nr?"m…¹BÏY?ï
ºR̬?{¶[ì"X?|¶zcš@?c™ã]g5?•0ÁV¡ÿ?ySÇ!BAGN4FGL J1248.9+4840¿¬äbÄ!@Qý`éNäÀ:½´ò»sßÀ<Ã9W9¢¹@=x±"ø@2™åﳂ?ÂxÛ^?«
®e?çˆäu_þm@)Ùçg'Æ¿åfH3ux¿ãn¯«SÖA¿æýh@[9â¿áV¨ž[¿ïΗÝ×·¿ï׌CoÁYAGNbcu87GB 124632.9+485605?ïî˜)8‰?wZZÆ e?A¡¯ûô?TuŸšj?Yÿª{EÉ?r§ú|%Éø?ïߚóiwF?oöc¼@w9??ÜÝó²?KÅ|B×h'?lip˜Ùª%?k2¾kҋ?ï¯>CÝzo?zÛ3«·?W•æ¾³×û?Jö^hÛ?=²7ª!5?zD·®oL?ïïƒmÞ)ì?@ŒGÿ^.@?I«¤—$Ó?0¹Ö3¡ºí?T#Q¿Áp«?9½ìb'm?ïÖ/Ûv?{é(ýjŒ?W›^"D­?^¹ª3¯U?nAVò3p?v‰²€±?ïœ}RwWa?‡Cò›û?LŒY¡#T-?Yõì
ì¡`?‡åń=™?…Í8T¹‰?ïYýߋ¸¨?‹[užG?a!g¾áÞ?YHÌ®?'œ-h³?Šœƒ%[P«?ïÑH›¶?aTÈy‰?bkíÄ'?Q»Òw˜Ã?lyt¶b^Ž?XðhíY&8AGN4FGL J1249.2-2809?ç8˜V'L¸@A\ÂzcÀ9óšw+À<J–6—l@4žm=ñ@/»õäô?¶ˆWQölÙ?¦
L46?ðÐÄ©Ü¡@!åÆüÌ¿âÚ%æC–X¿Ûhfç¿å&ýšÊò¿ÕŠJWu¿ã-ª}l'O¿áž¨âŒÒŒAGNbcu3FGL J1249.1-2808NVSS J124919-280833?ïÔçP×?dÄB#¸Ú?NÑñ#PÄ?=ˆC_r^?q²?Y'~´?a¦˜Q;?ïڏô\ç??qŠ/sæ?F"*Øò*ú?Pýû–€^Ü?oËËS9\?kŠÁáÁ?ŽbG¸?tåßÙG.?\«"¨›À?X:[5zÊ?…G+à
?s<þ^ýRÝ?ïŒbk|r9?b€Óú9~¾?lGòÑ!ÿÝ?I y7'^?…ÕhaD;å?`ˆŽ…dž?﯏·dýþ?qÃæØ:`ó?Z›†7ïÆ?IŽàh~?€È¡gðƒ?o£«:0Ëu?ïŠVãñ	?ˆLrÒR?\"÷
î–?e¾n?.Ü?‰åüè/×?"¯xgÀš?ïJ>ès?'9Ìñ0"?e˜J>[" ?]jádÒD?"«ˆëˆ?€ª˜ÕÜck?îÏã—k8?€ø ;u~2?'ÿç؟‡?i]:¡ô'v?œƒ«>ßC/?|Û3çëæˆAGN4FGL J1249.3-0545?íëçH'Ú§@L"V!uÀ9ìfknããÀ<)ñʳ@°5;Ì	?þ°ÆÜÈÃS?Àßäׅ?¿|F¢{Àk?üðÁo¡y@
óÍ]ìDa?±–!êá_׿҃Û!#f7¿ázá}]ù°¿ÝèèŒEô¿àáMø±W&¿èååvø…AGNbcu3FGL J1249.5-0546GALEXASC J124919.46-054539.7?ïø#}wi?8ÇøãÎÒ?0ŠjI?#•r¾D'?G»¬¯€²9?3yÌÌâÿ?ïÛèëÞ­A?pAT¡?C-ºr '?MOJÇR"ý?oK¥¾í›a?kgUä`W?ïÄ%"=0|?c)¸út³+?RJpåcþ?:Óù™`ó?yZÒ¨¾®‡?b•,v"k?ïž=Z~{±?`œ¯ZÄoM?aÛÒÑÿ&?@d†(M?ƒùÉZ~ˆ?_h•l¿?ïôÈ
舷?C`þR[¼??€WTF?3¹¸ËTr?M\¡,EÅ?:ŸCÌ»^€?ïâ•O̶?†ö™
8Ï?VD(z?``0Z#¡?‰>ØðÖô?".´ ý%?Ëï#±?q
ûIñ"?ZÄ¥ ZÛ?J. º)0e?"F¸Z«Æc?o?™•r+?ï^×HH;?}ÉÉ$³%ú?uÃZó‹%?\¢PhHvæ?šcN\nß?|ï:ü¦gAGN4FGL J1249.8+3707?ãñ—"h@Sÿ|E˼,À:5áŠëÀ<ZÝÌÏQ@ —øo'ßì?ú¤Ò—çè²?¾š½°û
"?»ÊkH£\ç?ùkøáþ9@v[»¹f?í÷G"êp¿ål­byFé¿Òv2â*'
¿ÆŸiýŸ¨|¿á¨[ý¿Ü'ÁM'AGNbll3FGL J1249.7+37052MASS J12494675+3707474?ïöVØA9?nO_̉Õ?#]Ìâï=?O}6ô?PçG8*Q?n:ÿˆQÄ?ïàH•£ž^?pÐ!¾9ä?@ÓèÎlù?LNîÈó•ä?k'p`üÌD?mŸc"øx?ﺛ!Y?o&d•AJl?O8/¡ˆØë?8ªãý@·?~Ëi?²]?n{¤µb=?ï¢>"R¾?c½Ä¶ó°ˆ?^(_2~!*?B+&¨=?ƒ«Rü¹?b>t¤&™R?ïõg"ÀšB?Ah@Þäƒ]?.¼zä9e-?k<Žt?QYIpì?>þ±'˜‡Ö?ï˜×wÿµ?‹ÑbßÂ?P —ÅC'?[´öy?‡¶Žð@?Œ2šTÙ?ïvI0S7"?ƒÆ"òkí?U´Ð¸ú,?GSzm¡2ù?·ԉÑó?ƒn8/Wïž?ï€Vã?€¼Tùa?qÜì¦t?\¯Š!Lšÿ?™ÆIö¥* ?Ôç"6OAGN4FGL J1250.6+0217?åD,ÊZÎû@PJ%®æ1ùÀ:7Faä ¦À<[DÐêh¿@Ÿ0'ü?ÿéki¦X?½e?½I?µô'žUk?øՐÀ­Ú@¦û˽Ù?Ú¿†ÞV&?ß¡B‡N¿äƒõ¶6ˆ¿Ù­K6_¿åÍF¿×ñĿُ­‡'›AGNbll3FGL J1250.5+0217PKS 1247+025?ïȎp?bòVæ"?Wðæ™?CóU<€ÓÚ?uöÌ	4Zp?_µF?/'â?ƒg7™º?f*Ú~!'G?m`^c/sº?'O}'k±?{kyä[('?ïvÓ଎?uŠb_"¼Å?fô0á?`@ÀKeæ?ŒÊÊÐ.'K?rÔÏ:f^~?îAö×à|?~©íäô?›ÄÐúºãð?vï©c@¸?›ün('>?qìÜÀ•pè?ï}ipÐ?ww×3j"?lãs×æú×?Z·Ž~]Ö?‰l¾ó"íF?t^ý²bP?îëCЏO?œŠ©LüP?|«¿'ôîÛ?ƒSœ—©â?›l–!;ñ?•ú¼(w´?ïÑ7·ô›?…yƒ?3Ha?r,8I?e.ߤ³X¨?šÚՊFч?'ÂgN.ë]?ëÅèx鏕?•Ââ²?°}@ÿkÞà?'Ý_6ßI®?±S{8Ù°ù?‹"þü'™ŽAGN4FGL J1250.8+3117?Ü8¸`â¡@UuÎ1PÚäÀ:½^¿¨÷ÛÀ<³ùJ÷@½ënM'@dà?p?ň#û\Ø?ÀÇ`âÃÚ?ú4Q%Œƒ@—멱¿«?ïéæ]Â}é¿Êp¡Mm¿àÅîÁ껿çoñ)£g¿Ø§9ª€¿ïÿãzŽ;˜AGNbcuNVSS J125051+311706?î\-–ä0?¾Âïÿ+ï?hT88Æ
?~!ã±ÁÏ?¨¼q_
¸˜?¾½*R™?ïÔHÒ+ÜR?ˆÞ8¿k
¶?C:î?Nªê!ï?stSh· ?ˆ÷ºý'?ïhýrº=?†®{ܺï?__·À?cëñå¯?ê`l¸v:?†Eadów?ï­;"x?a@‹Bo?k+£oÏÒV?Q0[!lÁß?{Ìd![¨?\0ùÔ¹'?îՏq!«K?ª;º°ßi.?rK~x¢œ?uÔy…M?x? ]¨}'Eö?¨àМ²u*?ïiŸ:ÀI?"	uésô?Yœ!ºÍ?blÕe?'2V£×‰_?",õCëa?îìøM¦si?'ÕO·ª$!?h[°%‡Y?i¹I9?ŸU€I˜Mµ?'6nÉXÆb?ï' 2÷?ÀØÃh.™?€:*z[ø?m?d‹:L?•"hPx?{ìiǕAGN4FGL J1251.2+1039?ÖÚjŽXÉ@Raž­ÕÁÀ:È_Ñ÷®ùÀ<Ûž ç×@å•á"@CLŠÅÁ?ÊC#–21?³Øj9ڗ;?êÿ'>‰(@y	ڛ?ÌöÄŸä¿éØS³Ü:ÿ¿Õ—zEˆÓ¿ßѾmþ¿äóUÝ­Ô¿ãØr¥®AGNbll3FGL J1251.3+10411RXS J125117.4+103914?ï"-ø€?µ¼»â¸ª(?€É
f¤0˜?µ>ø­?|Vé16¢·?"þûß!?ïÙåêގI?r1‰]¶èS?ABÿš°ô?Ku"ÿaôÿ?p䪟à_n?p¯ՎØ?ï¨à,Åá?q¯—·‰#?PÕϤžRŒ?Bâe?ƒ­;3{Ž?pûâð•ËÏ?ï°=¿i?[ÂÓ¥µ?[m;bnċ?;?Â²?€'èÈkí!?Yf4œ§±ƒ?ï¡ÖéӐ-?ƒÝK`€½8?V©Ôž§?rVÔ|‰]?"µØç>?
ÜPó?¢V=?ŒÆÀüÜuf?Qu¬úÔWë?ZÄë*y¬?Œ¯!ܗǽ?‹üD,(?ï@‹Þ?…\… —£k?ZÈû)'%ê?_«
¾9K"?–AôŽ+§?…hïV?ï_žB˜"?yúÖы?m²D‹JK~?T±Û²†?˜]íþÑ8?y:½ñˆ³AGN4FGL J1251.3-0201?Ñ®¹ÀšSB@Nl)Ür\À9çÆaxÀÜÀ< ªÍÛÁ@Wš©+½?ÿ5}?Æ¿m?·íå᛻Þ?Ãð\žçaN@
–Õ"õÎ@Ú\`ˆ×?îÃRЇlp?ÀÁûxö¿àÖ8¡1=¿ãh&à>™™¿è	 B*Fû¿Ü.]Á&PwAGNbcu3FGL J1251.0-0203TXS 1248-017?ïäa±uÙK?yOGW)Ìö?[ü†cÐ?væMìbåa?[@…ª?`Ç{)ñ?ïÜÎàM]+?pq<Â?EìþÃg?Píßct»á?m¶Ójb?jˆz?ï}.Ñà³?…iÈ°-eÜ?|)V…/?"˜‹¤#æ?'¤õªÕîÂ?w'Ðì¢n??ï¾@[Ԁå?\@'̛yA?]ã‡2;¡ú?B€1ѝ?yfð[¾ˆå?W'NG9é?ïä ;ŽC?]UÏSb?W¿(-Hs?NHû"ÝvŒ?`Yç†ó3?Rã2âyá?ïŒTÝ°}i?ˆ$pŒTîŒ?^¼à2g«À?k›âç›Ñ?‰,"Âü%?…"$'r?ïÛ°îº?7f/áy?‰!4»œ?ˆ¸?£¹@?(-˜*?'ÞrLà?ïbŸÜ)?x³2HZ?p¸ñ
u?Y1â«ÿH?P«³vH?u¨F´ËAGN4FGL J1251.3-1719?К+¸žC@FÆ~¿"ÀÀ:ƒ½‹ç)À<0'½,EÙ@Œ½T´¸.@Rå=Ì?Åi ÕãvÝ¿¯C²¡To?æÈa-A'?ý"ˆ'ðਿã)ò­1&¿çôáSlŽŸ¿èÖ¨]¬®t¿ïÿþó…õ?ïÿ¬ž5¿¿ïÿ±%§YvAGNfsrqPMN J1251-1717?ïͤ÷×Κ?}î´>ò´?a‹ôß B
?o¬ÐDÑk?pg‰ZÖ8?sñX±œV?ïƒæ4ãó–?"ìV ¹?nßÀúA‰<?3kâ4"?‡N'~{Ú7?‰èû	¡?í߉ú?<ƒšÒõH?™à£ežî?"DZf"?¥<¡§ø?"fõcŒé?ïè[lžu?YküìK»? …@X
??#~òè›rñ?fœ?X0öÉ?X¢o$©Ä;?GqD?ˆ30c]
?uÄ­if=O?|ý'˜¿?x/S<­?	2ú@\î?îÓ`ÓÓÛ?ªïՍR?}]uwã?š‡'bUÆÂ?žOÙ
 D±?£2?'g%f?쁁¡ø…/?¢ËÌa`ûÀ? _‰"ž"?˜K`‡œow?³Ä.'6£÷?=¹íù¢?/:']?…\"j†?KûÕG…
_?UÉä:~¸a?Š^öԉäÙ?"ÌÔøBªAGN4FGL J1253.2+5301¿ïRCwàœ@Pö¾7ޔÀ8¢}À;`F'µ@F‰!|?þæ™&­ó?äè!'ö?¶Ža¯Ž@}4ßݵ@¨ªƒ¡¶¿´wù
îE˜¿ÓFšDšd¿àíA·Zu¿àVƒ?4{¿ä\¼>4C)¿äCëGWLAGNbll3FGL J1253.2+5300S4 1250+53?ïêG'ö'í?Z'`"áB??ÚZàµ?;½àµ×ôß?a½Œ«*U?V¹Zû?ï-òeHë?—ŽÍbÉÎÁ?|ù{yñz?‡¼?ˆl{?"Z£X—î4?'œÂ½0d?ïxÑo#­?ŽMXþgÝ1?wÀSKe[à?ƒHrËԞ?…ë•Í¢®Ã?†¯/ÕqW?îZÞdò|?ˆ|, oa7?»udð•`?u°ÙJ¸K¾?¡ô_±ð"?'Z©þtú?ï賚÷'ž?`ïOKŸ=+?7ñ$tM?5ªOdŽ?^?dSî´ê)?_\Ëé;-)?íǧç)?°A¨›.?•®OŽR?£êÄÿTݞ?©Ï,ù]O?§jQYCP?ïg¸'qö×?.O™|Z?vÝ6<€ ?ËÍ&¯?Š£@?í÷?ŠŸ&ÿ—?ì,"fñ?? ÚTm;Â?¢Na5DÈk?Œ;½—áÅ?µt¬/yã?œUuYF¸äAGN4FGL J1253.5-3934¿Ëÿ8ÔKµû@7M‡ø‡eºÀ;Oô!¥l6À<­qGÏ¢@"RüÎÈ$œ?õ»
7 '¾?×(ª.'?ÞBãÈÂý@\ÝF—"@hU¥ÎÜ¿ääáÞ?¿ð?ð?Û襁6¿·d^ -¿æºÀZ΂¯AGNbll1RXS J125341.2-393200?îK:CPj?½F‹•‰?a2¦O;?vá Ã!Xç?ª4ý?¸%?¼¬ÍºÑC?ï¶(¬$>V?xgSÕ?Y''Jñˆ?e"ä¥b?~‡	J1̉?|Lg¡IÈ=?ë±Û«s?±3J(néU?dº_w2á/?q«&Œ—4³?Àå§Ö"o?±/s€UOé?ïubéÀ_?"&¯
R?E®F½€¤P?8Œ9Ö(?œ#ápB¿5?"Jܸù>?î2¶?´6‡% <?cµÀo›=?a˜¹svhÁ?«¤l³öä?´%Š*]C?ï;Ø÷äŽÇ?˜§"¸Nà?kü—›W?€bècžcm?•^K«HD?"R?§…¡‡?ꣴ¾Ê;ß?±>5³<Ä1?b‡Èw"?máÚ*¤]‰?Å(®æÄ?±Oþ×B<?í|w'÷d?¡Vœ¶,íâ?WžLMà?Z'Rwî½?³½ÎÃ3"?¡K:›DZAGN4FGL J1253.8+0327¿îMv
"z@P"3œ¾àÀ9vZT	lÀ<á¦x¥-@—˜épq'?þ¨S¦pA±?²\[J©q~?²ï'ó²ê£@ºÆ:"‰@ÂÂ¥V'1?ïæfÁ«¨¿Þlâ×P3¿ØÙL!–¨£¿âñµºa¿àajþütÛ¿ãIsÔ
3AGNbll3FGL J1253.7+0327MG1 J125348+0326?ïÅÞ¯U÷?eÓaÿµë|?Q÷nÀ3ؑ?A®Ê-=?x'Ì¿Œ,?cBŽä‰h?ï­G¼_Ë?'.Re£>?\pï!z•?f7#™Áic?åd?|ik¬1?Ë7Ã?|I&½îˆj?e'Noé?lNÿE³§?‡Ï,ªVJý?vHÂÌû¿&?îAÝ0$éw?«?ºzA¿?ŽûMъšÐ?n
BÑëSx?¤#Y…>â?}m+AÄ:î?ïŽ6ÅÂu?|lÁÚ¸k??b¸¥A{G?SN*Õs"æ?‡ö/×Ý?y¢qŸIšÊ?îþ_«P.?˜Œq
M4?s Us ¢?{¸pá÷ѽ?›Kõ5œ{?"ÅžEªøõ?ïKæ³RÓ?ŽÛGõô²?q– 4Ë07?pã»?šû"f*ƒ?Œg–ž.Ø?ëÇ
)¤"?›·.­Ñè?¡Q±¶at'?…!W?¹¾ÑÊS?—èø;¬‡AGN4FGL J1253.8+6242¿ïì­îg§@K5ܜM©À:YÜë(À<Ÿ!ÿ.Hé@ì˕j5?ÿRþûB0?³Dç­†?—qd¤ÍÝÍ?ä
*àÔ@´@»ù¨M?ï§0ü!N.¿â®¡Óú¾x¿àý¢È6¿Øó"
3`¿ä¾‡Å[¿C¿Ú†«ë«µ%AGNbll3FGL J1254.1+62401RXS J125400.1+624303?ïõ,¡b–?H­ùˆ¯Í?3•uUEú6?'døðã
?PÁ_üðä?Dínã?ïÜ«æçïØ?sh2ÿ??öXúmÑ?JV)'?ä?oUN6©ë7?q¾tS?ï¤þŽÞ!*?€0i ÍLq?P"}¹ˆß"?E|k"z?"­Ì'¦q€?€ðŠˆ°?ïãæwvaº?I±Më®ëq?MH^Zé>/?/&X0®Ö?dÇpÇ/U`?F¼KVû0É?ïë×
ºË?`8jÝÊó?BT'H€n??W¡©¶Ý?_'›;Žƒ1?Z_IŸN§?ï•ÑTŠµ•?Œš°‰¹ì?R #ù9ÖP?[æC˜'‡?ˆG¦PÄæ?Š«ÚvÊó?ï_rÆã?Œ35©³'?X®SÅ?Vn—}'Þ?'†Ë2YH»?äK/–?ﯺêïo?iÂ)à£?d\ÈÎ}‹x?MN€0uWÐ?}ô&+X‹l?f{Lñ#AGN4FGL J1253.8+2929¿í¹k½NÃ@Uä‡Tów\À;¦JœÜDÀ<èdØǬÒ@ —aºH9?ô‡™Sù?à?…¡•ž?ÕÜ%³î¯?ó¬õ–ðqî@ Ü&$?ïúÁ.ˆÿ¿ïÌ{n5gÁ?è¨+b"Y–¿ÎfÆÞvB|¿áŸÂ¨†œ¿à×QÄòAGNbcuFIRST J125405.0+292708?ïq-6;r¿?£cW¢°ÿ?`šV˜"??p*ݓ·^ÿ?ŽÕýÕ?¡Ÿ{sÓ\??ï‡$Óã±/?¢~°Ü— 9?_ÞvKŽ©?qtûÀ¾2?Š:ü8æ–?¡ÈÞ{ó¹?í¾Ž9Oh.?¡ô¸wuðW?vh±°?€+I†'%?°¥%S•Œ?¡ º:òò?ïU"'?'"®²þÃ?W±ÑyOç:?FKH7ÓT?žBÑ]õ¡?'deB?Ž¸?ïPª
ÉV?'ÀÎ"[?byQßHŠë?YÄ <sÁH?"›"†åUè?'!Ûøçˆ?îÊry'ˆË?²È)èÆMc?oË«1Ò?‡]h YO?¡\²úZþ?±ç‹fÿR+?쀦<®ö½?©\»Í!†?qÃ'øŽ'ê?põüîiï?ºÞ››^{?©/ìZ y?íÙg‡Î•û?žDt" 3?S·†ÙìM?S¸L/T®?°è äwÊx?ž/Ú¤€ò<AGN4FGL J1254.2-2205¿â{¸²…ñ@DcÖ¶Zš€À:I}.ÿÇÌÀ<HéH-–;@g:<fã@	ýñ7?DZÓ!O°í?Èðužg´š?ÿ|卍ó@
Ÿ˜^†;?íŸ9Q´~¿Ý¯Òò䏿â0"刿àµ{!	¿åI¾ RÔ¿ïÒÁ££Þ—AGNbcu3FGL J1254.1-2203NVSS J125422-220413?ïÚ¬~g~?qÐõ`M?OÔÒòë¨í?R‰'—WϽ?mõ=>?jÄj(ü«?ïÊaz:Ñ?sÿ÷RüŒ?PC«Øas?S€×ƒš‹Õ?v¾Wÿœ^?p"ÏiÚñ?ïo©…õÎ?‡NÚ;qÜk?e
"Ùìý?g\4á?ŽØp³¶=?†HJü»mx?ïàpî¥?o{ó¸]"?vê⼗-U?QSðü–?–é981ª?n'Þ'á?ïÃÝZ8°¡?kÓø3±žû?V/ZŒA°?Iœç·–öC?x…|ëÞ?hÄòùµJ¿?ïa«ô
O?™%ƒ<ù?`²["¥‰™?eÑ#¹
«?'´5÷ê¤ý?Šõó\•7?îêw(ð(
?"×=l'?xç«ØÆ?}mß=}
?œw0(µØt?'d¦îwߎ?í•ÇüÈ+í?‹"ÝaÿÖ8?Š:«©dÞi?mbôåÝ?°
j¥ÛßI?Š8LýM+AGN4FGL J1254.5+2210¿ïO𺁊s@U@'(bõ™À9ÊôWÀ<UùK°Øz@¢v Ë@£iüóÜ?¶¢`<«¬í?¯«þöë"H?õUŒ·^¦@…Í»Š/C¿Î·_}>@¿æÕïUÑ¿Ùý"$½O¿Û…íÀ7h!¿çO;Ý%àd¿æp÷б^AGNbll3FGL J1254.5+2210TXS 1252+224?ïõi–¸?EŒßLö9?0J#$"ï¥? 2žÞ©?QKRà1ä?Cw¥
¤?ïÐGµ:"Õ?yF¼Ï›ã?I1	1Ô?TáóÌR?ô?t¶¦†P·?vúøÆÞ?ï¾ñb¶â?r•}Ï¡?Sµ·AÖx?_fM'{¥?{™àôœ~Œ?p€GUW‰ú?ŽÝ‡?b_Møñ?á?llrÙä$ê?PVÁm¨î·?#¹ø?+?]¶ðŸiW'?ïðJÍb?I¿¥ˆ—i?:ùËÉo²¯?(]É×	å?X¬Í•˜?FÕsf‹n˜?ïw4£Â?•8ú¾Ó^?Z†[rÆ1Ú?g…ÔGlß}?Žâ/PÑW?"eU	ë½Þ?ï—柁+?{"ŠR?Z÷7/õB?\Kxäï3¤?†ÅYV˜¦?y[ÿÿâ?ï|ä­?ÚŠ¦êÁ|?ë¬"#µ%?kúüÑÈm@?–ÇšMP?}pª½!lAGN4FGL J1254.9-7141¿¦vÃTù¸…À!¥{"ÛœsÀ9û<š»ÉÀ<³"&jÎ@l·2[ÇÒ@>öÞN«?¿j%®(ó?Ã?áD‡@làÓêÎ@®qLÉ\U?ïòr®sEr¿ÜC¬ýúl¿è$dIU´¿å{ඎœæ¿êˆè""©¿ß'ÿùtöAGNbcuPKS 1251-71?ë×(¶E?Õ¢oª÷~Á?±èѬÙA?ÎúߜT¬L?µÐušš?Ð7Ú|¸¸C?ï 2Ӛyò? £CÏ?F›":'?c;6•pó'?›E,ª¹ï©? 9&EDZñ?îܸø&T?Xí{?~R³|§@?€RÚ)l	?œÔ4<v¥?‹å3EÞ£½?ïÐòNš"?Uh¯…Uø*?H…4Ƅ³´?+æI$WÉ?tv2Yé'?Tӓ9Ôõ'?îÁÄÛç?À^
Ý
a½?ˆú˜­£vC?¯ªMäíÞs?§õ=‡´ ?½Òr†¸Ê?íTèojœ?¶è©Ë`©?VÊôzÑ°t?p¸€Æ1­?´ý²©Û½?¶ë¢µS?íɊ¬'!?œù£ÝyÊ?ŒÆöh	{??‡Ìf'´Œµ?¬5—¦E?˜]•KR?ïceÂ}"?v–£}b?eHÁ	ט?PQ‡x‹à?ê/Í;û?u"$jLãAGN4FGL J1254.9-4426¿Ú3Àá0@2lYtæ[êÀ:DN®¹¼OÀ<;hë{ä}@vîªíÿÍ@Uçþz¿?¼ýòÆ¿‰B
ø'´‰?ʎ"õ"@ƒái\æ?ïèÝ¿cW¾¿á	Ê^ˆv‡¿æ`Ÿ¨žð¿åqž½c£¿Ö5ÿ€Ô%Ý¿ïÿúVrÓ\AGNbll3FGL J1254.9-4423PKS 1252-441?ï'Î/½ Ì?€]¼ÂÉ?g>Ø_'C?XÐêÊSí³?‰|¾Q¸?}:Ž,ç1X?ï¦Æ''è?…³['<1?VÞiJN?W@г?ƒŒÚý`?"ÚÉGÛ¯?ï0Òu®,ú?ƒq¸+6ƒÚ?nÂ#%¡?d~rD=¹?–
pÂ:³?¤o#
'?ïrÎùš,´?iþu1'?f`÷B|?K¸Ôý…ÂÆ?ÅiQxx?f•Þ›x¹G?îµÿ¶®Ë?™©XóDx?€4€¢6X?r…D-™†? 'æú"òÂ?—Ú
\3'?ï1ZoÚzØ?š8`½¬Š?eÜî¸ñØ?xGýE¹Z?—4jÍÊ?–Ç™۟?îÛÂ^õ?–;­…RÈv?"{'aÅw+?}Ùæonûq?©³z‰ùè?"W/Ó—?îXØHÖÞt?†=Ky áÕ?€þ²ù–J?l7Ò~Žb›?¦2β ¾¶?"¡@:+mAGN4FGL J1254.9+1138¿ÅŠ,Uë¼I@RŸ÷ÎÙ‡À9ýpƒöš&À<;á~4¹E@…6»©@õ–AöD•?¿Rj,d¸?ÊÐfŠM¡?ÿÀÑìÇ>@
©ØÎã¨[?ÙO³œz¿ã³ü†Î»º¿ëò…žeh¿è¹F¨Zý}¿à×Ë~3Ó¿ïÿœ,ñВAGNfsrqON 187?ïÚÎî?"¹!4³.ú?fź¨h°?ŒÚÚ5þÛ?_ÚØy	su?y•¬éÇHB?ᆳ܋uƒ?{fçð¨•?U'Þ´ú(?^ÄDJ©£?{DZ&Ùßã?vOžô+qW?ï7bµyý?–6Ü·°Ä?ƒþ™1lš?†yT`Ǚ?Ž(å^"?"{½ª^ҍ?ïkøÃíø?gfSÅ?w»í"¶
Š?a'ox8kñ?yŽ"II?Xð
9ê?į̈:ØTQ?sSì?nÍÿ&ç‰?k…à-cN?d‰ÅùåWà?a¸ãRt'á?ï3PÐä×?"›&30ß?jí6‹—¢B?sb	ŠÅM?–8?Õóä?' üNð~?îvz=2æ\?™l<çø?—ùÕb€O\?"¾šíÈ+?™6âú'?‹ƒFW°Ê?î0ÄelŽ?'g°ºÞ¾?˜ÍÍví|ƒ?‰â®‡þ–½?•,ú­#È?z¼ç¢Ÿ%lAGN4FGL J1256.1-5919¿×
ÀÒÇ@_0ÓÊÀ9Ç\ŸTÀ;Ï©mL3µ@ uxj…@újÊy5v?¸Í¡Þây¿™4YªÓ?â#Aî·Ù @B2<h;(¿ï¼IýzÂ?î—È©Q'¿æµLG×/&¿ÞyÀGƒL¿Ý€&Ö@¿ÞêiÀ¸íGAGNbcu3FGL J1256.1-5919PMN J1256-5919?îx'"Ѽ?"ãpAsÒ?kq(Š+s?`"çzb?¦ÍF¼ŸOˆ?"GØÍ/Iú?í7'b<Øp?²«m¬€Ò?aÇ"µ×Ó¿?n4‡æM°B?µµ³ÙöPá?±…óBAü?íŸ «‡%?™f¬þ¤?€6Ö
º¿?rúߍ¤Wà?±è+6µ?˜ÓÁ˜7?îJò•fâ–?€HÙ«2h?|^ï­ÚÆ?[†lOf?§Äø´Z…Ë?sx?{CÚ?ë΢¹?­;§ e¥?Ã¥H†Ñö?vi'>ƒTÓ?¿R{Lý^»?¬_89vQ?èº-t²›?ÄX	ñ	[ã?{ªIu:z?Œ'‡ÁE~?Ì9ùdÊà?ÃØE?¾ö?éi=ˉ?«évD¸"E?'ÁÎóÁÎÚ?ƒf>㔉??Çf!+7«?ªu€ÓßE?ë²4Ux-?˜?hbÏ_?'KŽµ=?{Æ÷žG'?½ÊHšðÔ
?—s‡½ø>XAGN4FGL J1256.1-0547¿íðóô³›@Lˆ'ùD$À5…¼ÇœdÀ:}2ñÄÓÚ@"¿/üÈ@'d¼B;?y@X¿	?²Û''ãB@0­ÇGQÎ)@$ ?ö¶¿ËDYv=ôØ¿áVƶ2W¿å='AŽ@¿äsçŽ2׿é=Η¨(¿è·_èã«AGNFSRQ3FGL J1256.1-05473C 279?ïna»'ò?'@›ÌZÔ:?e'ÒUihJ?uÓ@ù'EU?Ü©hã|?xA—œ?îÛä6˜9ê?±t™"m7?†bÊÄl¨‹? ŸMSç?™RÂ+hv?¥ð"¤‡K?ìo=8€á"?¯Îø"R—?—Ç'f¤˜´?"ZÔP¾x:?¶"1¢½ÄA?«£-ìø;f?ﵧZó?€vÄ|ñ?hÚªÎ"ÌÙ?n.OG?yW?x-?uX1¦)?í«mæ|:'?°
¸9Ð?h¦qòHJß?ic"³®~:?±ß]:ß3?°`eà{?퇎Æ.½?»$¯%á«?š?'v›£ñ?°~VëÞR?ªgJäk)8?²»T>ƒŽä?ìåC‹Åñf?­7œŒX·~?'dyeíPÃ?"Eo6HÛI?´<ÅJzâ?ªxU4çr¨?ïr֝lH?š­ø#C?}߀6þ»?".±n5?•‰íRtB?•Ç΄AGN4FGL J1256.2-1146¿ïêO¦í{@IŠ<æÁÀ9r‹ò)ôÀ<øð@€-.â@§?þD
Öó—<?¯@ÄkTa×?›×Ù½˜sÌ?ì'Õ ™@cO•Gû¿ãèÔÀ6;{¿áKû¡K"©¿Ø}ŠDg
*¿à‹ã˜Á,†¿Ú…뜛¬™¿á¥sŒ¿–ƒAGNbll3FGL J1256.3-1146PMN J1256-1146?جÝw?ŒöÄBÃ<?_ƒeE@/?`ƒiqR¼‡?‡é©p_
=?‰1µ啚?ïµ2,æF?z†æ(àiM?Yx—®lka?_p¨£šÈ?Ïá
?u<°Òž²ƒ?Â$R?–¡¢ѶÔ?yNwNñu¾?zQ÷ÁZV?¤‹äöË_ ?•g㿳	?îdøªÌø?'Ð'•Þ2­?€)K
ԃÂ?a‰(5½Ìá?¥¦"³"?o)é?ïþÂ#Œ³?{Þ¨Cš?r"°D¹"ø?dø–s,D?™ºû¨¨6]?¹,-›É¿?量ôz™?•÷L,r\?jÙ¨0_X?s6díGÈ?™°YÄà?"Œ]¢«?í`Ç7·?¡u‰ZeÍ?"K×ȔÚ?'ü«P?²u¶ä£Æ(? [á	<64?ì3ñÀCŸ?ž"ç×#Å?'Kóás(ë?|¿¨Eß«?¹Ô+{XæÌ?›ãš®<tîAGN4FGL J1257.2+3646¿ïRX¦EŠµ@TçÿX:TÀ9à?d‡À<gñBÍÚê@1ÆöI?þ¨™Fƒ?·›"™ÐK2?¹v´è)ŸŒ@Ìø×Òª@
ö8#¿çtØïð¾D¿×šƒT]Ð¿à¾V<"¿Ú«
š¸¨~¿æ~VG4qø¿ápq·Ó@"AGNbll3FGL J1256.9+3649RX J1257.3+3647?ïø€³Úè?5¿'aÏT?&çOÞo?Š£~äL?HCpύu?2ó~MhØ?ïÒÀÓn?t×zµ.ɸ?HׯO¹ï?S¨Ï(@?s…xí÷õ?q¡ð•ò¯?ïÊò¤o-?[|µgëH¦?P¯"Ô«'d?<×lq'§?vZäòB[$?VÞ¦œ=	4?﵅ò.z?Zò6üÞèÏ?ecßd0VŒ?F½IðP?z‹£â?W¶PeÉ`?ïóô8C	â?BLxÎ=
?5B)³MË{?#|Ê~¨›?RÇÝDŸ-?>‰=žv™)?ÍéÇ?ŒÈöÒ¥kï?Yá–9¾?c­"°šçH?Œ¥PE¸|ü?Š¿Þ""ûæ?ï§öí:^(?pymÇ\4.?Y¸E‡ÅÅë?UìÈxÓÉ?'Ë<Ž?mðÃG£?ï<{LbÀP?|f™Pz?zS!¦ËÏ?b'H—ìé?'ÛÎ
ڎ?x>n‹ˆ
ÈAGN4FGL J1257.6+2413¿æTiõÎ4@U±Eà´áÀ;̀üê¡ÊÀ<Ûû()êµ@"1Žw&¨
?ùb¡ Ï?Ó¶…">C]?²Ýí§^Ô?àyt*tGÐ?û¢Ü)T?Î<©Ôz@8¿í¤u•®RŽ?ªá¡½våÝ¿Ú
÷À@wi¿zQ–åNË¿á\ǶãV|AGNbll1ES 1255+244?ï>œGô¶?£ÿP؊›$?Cÿã›gL7?Açy?Ž?X-Wjä¿?£à¥3æl?ï™´hõ.?«Ž.œ¨ø?t
í·$°?…6®ô¼ÙN?š(÷s'?©߶8ª¤?îJÔQGè™?™žÈ-"C?`/Á'ü}?ZMÄñAW?ªO¾ÏÌ?™ožu*âG?ˆ¤?‡ëEÁ|Íá?Z… #G­?J?qÖÕËq?¦¡&;4%Ð?‡Û]¤Äò˜?í`´1Ã?¹ÙæȘ×õ?X'¦}³'?Y³´mõlÏ?·šïýq ?¹²GÙfç?îMÑç`C?¾
ˆÃwRa?v»9ÖK2?†›å®'ûA?¬Ó»¾Žé?½jü<òð?ìó㪪?¤sòWU9^?eûǯ'/¥?gB¼˜ð!÷?·±	"Ÿx?¤QrZׅ?ëK#–!?¦d€ÐMtx?jÉ¥Ê!?d{±M&»·?ǬöÝ[T?¦CCKчAGN4FGL J1257.8+3228¿Ð'æ•Sll@UwîN&ÕÀ98dUêî À<	*	¾Å£@|%ÉX@À«;'?«Û¡&ŀ?ºS*tr×@µ›Á'@'ãçp'?ïÿîbHÊt¿áû–ä³s_¿äDÄU/¿äÚ
\ßÔç¿ê9yh¡ª	¿éN‰€Fâ=AGNfsrq3FGL J1258.1+3233ON 393?ïÞ¶*¶ü?fX÷ª©\?Gq…V8?Amé_ÿ~?kmtO½†?cŸ‹
‰•›?ïÙ$ByÖ?o…Oϼç`?Cí"yVcH?Nz'ˆ‹ïd?pðBãÌc?kªOWð?ï;sô]N?°¤å Ý?vZhxYÃï?|CÁ\Áuû?"·hÝE2?ãq«ž;Û?ïî^X©?Cëk½V6?Ef¡Ê"?/bøÁ`a?Xó]?@=Žyº?ï«`Û?ƒï&¯
j?XÅ‡bý'?Y¦~ÔyBý?'+"0Ý]¶?۝7?Xzü‡?ÁŠ/‹ŒO?XY˜ž,0w?i麾·F7?‰¶ÁÀU?ŒwljW?îÌúò¤ø?"Ô‡+Wò…?†WLºLÉ?‰"ÏX¸ëÔ?›4ûf;"í?'#rfrýX?ïÑKaË??aïâ[îS?\Hª«8¦?I¦ý'‡÷?pH$Ð"¦v?_8ȚJZøAGN4FGL J1258.3+6121¿ß.ã"ôÐ2@K߆
¢À;K›	bÀ<ò"Ì@"öàqšL?ýwœiW²n?ÇÉey¬iU?ÅÚyMBÔ?û$Éþ¼3"@§éÙM
Ð?í
z<@Œ?ìŽù,§'ø¿Èêû÷\ÃO¿Þêz\½p8¿äQÁÞÝ£¿åé÷ 54AGNbll3FGL J1258.0+6120NVSS J125820+612049?ïÓæjd´?n…ù?í?S˕ܟún?Gi‹­Á?q
ë²ëK?jÛÚö
¢?ï•_0DÉç?ƒý‡;[ha?ie"d¿‡ì?o~•âHí¬?"NÎÑ~D?{"aÓ©f?ï€.'/«Ð?wVÜÝE}Ô?gƑ'ÊyN?pÅÁo;l&?Š»'¹‹?pHîùW?îӚ£Ò$?~³ݖr—?"ÏÆ¿Q?v¯j¡Á~¹?'¼äÉÚ`?p:Ù_¢?ï°œíÈ+?o»y¼Ò'X?e,úQBÒ]?XBI‹m;­?}e4u)?jB/>Ô`?î÷1*M.?šE! b?wïõ;˜ìÒ?'[x²%z?›ÝnW6ù?"¥Iï߸?ïÇô ÑF?ƒÿÓºp·u?qŽEoC?p#©E½³,?˜"Ó~Ün?€þÜ"ñ?í^uì–@Ê?•xGåFì#?¢é',ø7ˆ?ŒÔû²wèÃ?§/ÇÔß?‹ñÿh(ÔAGN4FGL J1258.6-1759¿ê4ÜÅW@FkÇÞP'ÏÀ97-Xþž×À;êU'þ@'°«@ݝ«w?°n²ÿàå!?Á–€JGÖ@I¬¤j®@[Ñsz¡?ã·íu?¿Ý`¥\E{4¿åµÔ}›6R¿äýÄy¿êéý)‹ê"¿ïÿùStAGNfsrq3FGL J1258.6-1800PKS B1256-177?ïÏ9Ôbw?hȖ½âEO?d洜U¾Õ?]#C¯âÆ0?kßvÙ·R"?]·êÀ8Kï?ïÒcTŽ!Á?u/¤ëëé?N]Õèeî?XÜlïä?s³3R¯?rcVÑoâ"?ïi"@ö&?ˆI¡71jg?x°I¬ëµ?}+©H…¢8?‰cˆ"FÂ?'9蹧S?ïÖý}C͊?RÊñz‰ž?S¼Ø?Ÿ?9 ¢+™?ov$Zv£?O©'¤*¸?_"$m?}|Ð9®—l?sY
Í6?l­ÚÝöY¨?wP£le?tþ^£ý\?ïm—¥£"?'€÷àl~é?`åBiMøº?k6G\?0coë?ð‡îʙ?îôS~F?"§ÆT¤?"im+Îü?"Ž3½zR	?—IG]ñ"?ŽsÑ®àˆ?ï—À[ØÌh?q²&4m›?h×âǹQ@?WôZ-U?ƒÙðHÀIÅ?n-E›[3ÚAGN4FGL J1258.7-0452?¬‰›öpS2@LúRv‰ÊÀ:Úž´æÀ<_ãåî@!wãۇ$Í?ú—FBÐ?ÊRøur?Ìçø··;ì@Îå«Àä@‰þЪþ¿ãtyŸ(NÔ¿ïÿÉy[5±?ïÿç¬L#Å¿Öèq²Ë¿ÜŽòâ
K³¿Ý»u›AGNbllRBS 1194?3_J`?´ò4ݤ­Á?Y…Œ0ÏO?cO'yÀª?¥x@hîˆ?´¿Yr'7³?﷖N'çH?}Å3Ã[?SÞ_äo•_?]³U°HS?=@ÆÐN¯?}Î|rëœ?íª-g0)­?¥BrYÃÿ?\z»ö<ê?`캼ª!?²<¬–ÿéã?¥GÙÀ¢?îUÅÅØ£?‡b±"Ñ́?cµ~ʆ܉?TJ¿þõtO?©hK·Ç(´?‡øóA7?îBâFöMi?¬´(+¼H%?bpe"È]ô?[Uõmfs?ªªÕ8"¨™?¬‰\*ù?ï7Ã\¥a=?˜ÙìKì]N?d…½˜I0ú?qNs
?–vܾ"??–/"¬Ö?ìZ<\ä?¬¾2É3˜¼?e³ùÔ±4x?fX]ûc:?¾gNo­@?¬Óç1ø¬—?뫑ç|.,?£Îñ
u"¾?rÏå<шÆ?l'•½a·å?À»97ÀFé?£ž§ê[AGN4FGL J1258.7+5143?åÄríw+@PWÀÁü2À; ¼£‰ÝdÀ<¥~`X/l@1ˆ°h=+@懖ü?¼žWµs•¿·QԞ}Y?üÚÕٻș@ÚÉWLm?í}î¸u'¿ë¬dAÈø,¿è†çn2
¿Üë›D«¿ë/˜Ÿá²?ݘœä§´åAGNbcu3FGL J1258.7+5137NVSS J125825+514225?ïmÈV.?")K3?k<ù-œ|?d%qgïýý?©é5É8?'…¼OΊÂ?ïrÒõ¨/¬?"ƒ³UÝõ?p5{†	ú?…¨-† ?‹0"Ö^³ú?ˆÐŒí0;ÿ?îîG‡í¹p?'ƒj»Ý&¼?nºúž^}Î?l(AT– ?ž_¯±ìž:?þŸ
z_ö?ïkö:L?t&aèw(#?weKüN?aî¼äKƒ?‰®OÊrÉY?p³¯åùS?—1?§Id`6R?'ˆ™:º?y /Âí'?¢õ¢¤=D?¥ßtԚð?îƾ´õÚQ? …«@¯p?w¾HP¬åÚ?'a7bJ؀? œK¢+=º?œl•÷³?íÀÓÈû˜#? O"""'?yâhÅ-G"?vž>]Ë?°[;+
€ô?ŸZ›>û·?í—­EŒÁ?—u=åUê?˜?Á@d?ˆAÏTÒÅS?ªŠµG—e¯?'"¥ß\£BAGN4FGL J1258.8-2219¿ì³¬åH;%@DA¸d"À8ŒR7Û9À;‡Üßi‡ƒ@ÏZ/Kr@¦áÞ¬É!?¤h_ž¡?·î…?€¯¤@¶æS†Ò@ínοÁ!¿Ìl•?ì+¿â8ϟý¹¿åg­Ó
¿æZ§K39¿èꀥ+ô¿ëʶDËAGNfsrq3FGL J1258.7-2219PKS 1256-220?ïÎe¬é=Ø?f«¼5?Q·JúÎ^?Df¡[Ñ?t_aº²$t?dÌ95?x?ïØ%Yg
·?u•c"Mú?Cv[H,#?LMjz§­¸?q~‡í-?t!w°?ﳎªI·{?w$6>Î{?`Žà	?gÊÊ¥X?}ÕËÓyÙ?sÂYÜ^H?ïá7£|g?Q:yo¢æ"?Ay6²½õ
?+ÓX²NN?jjS]1Î?O†s‰
¤?ßËEþ?ŠÌ›ä€±?\è¥LS‹?XŽH±¸\ó?‰Š
õZ?ˆjBKÑ{
?ïr'œ…Õ?˜NdtÆ;é?[Ž…à›^?rÓ>•4Ú¦?íˆ™£
?–²ù">RF?ï ¿»õ˜?'®ªt©?g×£¸|îÉ?r»- q¯?Ú(ñþh?}øë›egá?靖zãK?r<"ÿ·c?Y÷ŸËð(?GµšIÕ?'^òÍ.?pã拼žAGN4FGL J1259.1-2311¿ì<-)ȧ@Cґ!%¶À9'u°ÐîÀ<
ìíԄQ@Ab…Ü#@Tò»sÞõ?¶‹4|?¥0â嬱?ëÝ[IŽ¿@O×X›Í¿ã‰è‹o4¿Ù£¤ÛA¿ã]'âïj¿ÚZ›WûQ¿å<á1ޟ¿Ø'·þ¯AGNbll3FGL J1259.0-2310PKS B1256-229?ï÷Zá_?;ìłM<_?)*š'î?†Ù
Ô¥é?K¯ñ'œã?8–øÎ?ïã&s\æ?lê›7Q?=ŸH֞?HÛrlöf%?i%£ÆÒ?g³ñÐÉN?メ4?orö'/Þ?[yõm·‰á?iÙë³À"?yØx¨æo1?bÚ×vþÊÛ?ïÕ¿¿óö\?S,|.ª…v?Ck؞8ô6?$ú
–è\N?r²¥
¨û…?Rs×;†Uÿ?ïôVƒð:?G[҈Iš‰?2.Êò\5Ê?#*:фZ!?RÇEœgåM?D
ddQ.+?ï¢4võñ?†À':#?Pi¬sëO?YtYÓäζ?…e¬ø´Î?…h¢,šz±?ï"'YÇX?xÛ£0ôx
?d'+o¼?o·3ÿP ?†7•–ËK'?sfýÄH:H?ï‹Äž¢df?sžþfWŒ×?Z™†}ÍÖ ?C۟Ҙ T?‰»§{þØ?rxI¤¤
¶AGN4FGL J1259.5+2332¿êGª}[d@U~ªâ—9mÀ:ÎdÒ°,À<D(v@Îý@¯Ígý?@ÍDƒ½?ÄBðëe¿³t¬¾ÿœ?íä¦Þ%»?ÿ.¾+Ê3?¿â‰€Ç»–¿æØ^NêÊ¿èïæb.ï¿æûƒ¶¿éO}¶åû¿ïÿò~#¿AGNbcuNVSS J125936+233047?ï˜ÂÔ¦_ü?Žó®*?t/ù®‰k%?xpáf?n›ÝJW??…ÌÀEQ"1?ï^
Lµ? uXØÅe?r²"©Gä}?‡T«Üoà–?»Aì?›Ï­ý©¹w?îxÊ9'i?˜ÈÅq<h?~ÁE5»b?~üШ}ýÒ?¤›5ú-›(?—Æù¸??ïN2·ð?€n{ÊWýÅ?"º{yc'M?q£u+]ù?"Øü¯Ý?x´L'Ä?ï"¿ r?œu¤a©ž?‰€lï8ÿÈ?ˆñ{ïè?1–

©?••ÃmŸã?î¡Õt³~?²[¨§T?‡U¸_È=?›Š/˜>¾?©t¦r?¯Ü:`è½?íibŸ‡oK?¢Ïuå?ŠJ¡Úrâ'?ƒƒ‹
ð©ã?±k–ÉRe?¢JÖ=»?썰Ñ)äç?¢†tbxQ=?¥7R64˜¯?˜ÂÉyí=?°öÐ[–Œp?™
è,ÜAGN4FGL J1259.7-3223¿ïû;có@>r螺jÊÀ9{f¶~¢À;ðítA@èU³:Õi@–ªú-´?²=å~I‡?Àf0 .H¾@
Ä.béÚ$@µ¬]@¢Ý?ïû)ƒ£8¿Û—\¨wƒ¿æW!U;œ¿ä]sYN¿ét7	‰¿ïùûn Ç‹AGNbll3FGL J1259.5-3231LEDA 4075145?ïÜ.L¢"³?`O" ?ù?RÚ~ì%Ã?LV‹g—?jdsà¶m?Yҝ*w"¸?ï܆pi8?nû	¶	)[?G™âSĐ¥?RŒ:)Ûú?m"ròf"v?hPé†Ô¶t?ï‡ö¢šZp?€M'r{?sOõƒË·.?xxßa
YÚ?"Z\èd?q>áÁ–WÚ?ï¾àÔmø?[¡å 3YÒ?[¨	3̈?@ów_¢?y¥œµïlà?X
4OÖ?ï¹ò8°åT?pnö`­?d»¬ƒtÜ?[ÿ?ú5¢?x©
}0 8?l
þZk&?Z"?"öÐYÞ¾s?\ò§©ßf?hƒ Ão½?†¹Ç8B¤†?òrÚQ¶?ï%žWþ?K•_
B?'àg•¯¹õ?'­Òðñ?'ÜWŸÍ[?ƒ§!+C±£?ïFjü‰d)?zÛb%‰ÞX?uÈ´¾Pñª?amB?–÷?'Às;ûŠ?vôRľKƒAGN4FGL J1259.8-3749¿ïûµâ
Ý»@9²c"úÎÀ9©N¬5}À<4\¬©@×@û6½\@΀ÌC:?²­¢ bl?sLù7üW?¿3ƒåþ!.@2Xª'
¯?ïé»ðÜvŽ¿àËXߕ&¿àߪõâoÌ¿á‹}w$$¿â፞¹"¿à®þúGAGNbll3FGL J1259.8-3749NVSS J125949-374856?ï¥ZFaR?‡oŒ‰•?Sièf²AÖ?FQó'1Eó?"<1PÞSƒ?µx¥Š?ïÙÛS"fÝ?q¤¦'LZŽ?Fè·!º`?Rüz¥Iõ?p5?|í'h?lªY-	wÊ?ï,·A†nU?'G¤ù+÷ì?Zì—iOç)?a¹‡nËo?˜ºNY¥ñ?'×H؊:ï?Hï?föÑ¢Yd«?gßVoÿ'?F–íh?†Â»¥'ÚI?d|耫æ?ï3ÙÚ§V?—jbÝ5s×?eDb™g?[NÛäÑ~?–ù|9S·!?–¡3Dd®·?ï˜^ú{¸?†>µ/&}?Uò¨çð®?d"‡—?‡)ìL>Óî?ƒíŽŸ{Áþ?îÝšœÆA?šD"lì®?`•þŒfðð?]Ûa&îѹ?¥èÆn]?™íœÑ˜K?î×d£Ì+?"+kÙ	ù€?~i#ƒ]…&?cjÈ]ߪ?y"¡W¸€?mÿ·ƒ®AGN4FGL J1300.0+1753?ȗaTò@T#ôörÀ:¶K̇,°À<|÷¤ëá@
º´2w@pÂàºÀ?ÃÆæþ¸?Ÿlp&궩?Ônw⏬±@›îÀèh	¿ì'+ˆDÀ?¢›+Ñ¿çØs>f6¿çE)Õ¼_—¿ïÊù=n˜?íýgŸKŠBAGNbllSDSS J130008.52+175538.0?琢€k~?ƒÕ¹níb?].›D!Â?]˜pÂ:m©?ú9}Ü`?Hcú+üÇ?ï®u÷S;?ƒ¸©Y'[?Z"@ŒM-î?e.q¦51Y?ú"Ú?€`åPX?îg]Ö04?™¯0˜Ùh?€òkt@"?}‰[°˜?¥M‡Þ‹Z?˜éU43?ï¢BìlX?i1MÊu?sʧZ®Á"?^®cA¤(T?{.7Hˆ.^?_ÉBt³Ìò?ï:ÒÎ2lS?•äîKç¿?pl…)ï?kz3o?"ž‹¬Úñ?"óFÈ·"?ï›,|ñÔ?Ÿæÿÿߌ?mýô…v«?yR2°?šlÛܛ]$?Y8§ý¬?í+"ÜyÒ?£2ªÖ—~?‰Ø§\¶ö]?ƒF›rEBƒ?³hD0 J¨?¡äBØiN}?îÝ¡K>³?‰ÔôšŽdœ?7÷Ïiê?ôç0?•¯Ûç^–?þà<¸AGN4FGL J1300.4+1416?ºLy•Ã Q@S>iƒQYÀ9tùòŸÅ-À<<Šk(m@_öèª"ÿ@†dÆS6?±—"–}/?µÝ';¦t?ûÌO~ÃT~@j«²¿ËÜNõÜeœ¿æ£¬!Üs´¿êHõ!¬‰¿åòI(gþ¿èò%ìù'þ¿ïü±®¤AGNfsrq3FGL J1300.2+1416OW 197?ïãhâŽøM?¡ðÂŽ¸?d+äS¦?¡ó‰˜þ:Ä?P׊Hš?B_«ÚW¨Â?ï­dÝOPö?õó–øðæ?_ÓéI£Ã¯?iPÅRúŠµ?€¬K†ð?|ÏG½ O?ï°S4ãêÿ?x[³ÒL_÷?c0â';8?pž•WA¼­?~>Y~ŒÓ?qfûRïU¬?ï½Â Îí?b=•$P'?tò}4'ïV?]3ž^¢o?hXd¶/â?K'ŠÈÍ?ïåî}í?_þ50«?Q}`-0G˜?Læ¿ýÄ¢?a¿a¾,¿/?Xó`½3—|?ïSLòæ¬?£_PJ)˪?t«×½-®?˜p½É?—ê ›Œ%!?˜‰d>Ú5Š?ï~éCiÐî?€~"æÊ¢m?oó/Vi¢?sߖ@…>‹?ˆHãAÚö?w¯G$¦?ï)N4XC?†@ 6ÊJ?'(ëÂÂn
?'Ç)(|"Ì?Z›‡Óo?k¼ÊðÚkAAGN4FGL J1301.5+4413¿ëx;DÆûÊ@R1×Ûô‡ýÀ;Q3Ï:eÀ<×ÊZ+Ł@4ºuÝ&â@i[»èxû?™ڇ™x¿ˆ»Ö
ù3?ǵ­áÐ*@/xº{çW¿ë‹hH¾µ³?濞`¨·D¿ç£õ¾¸¿×|ÅW7Ÿ¿èŸÐ_©]Ý¿Å[¿XðÜ÷AGNbllGB6 J1301+4416?ïî›Obz?RÌϳ¨TÆ?A¾‡<ˬç?8ÊîÚRI?YêöÏ|?N1٦⥬?ïÞqo®ä"?p#ßÝèc?@ÐÝ+:
5?JoÑÿ`?mZYsÏe?l°`þ?ï¥í.¹sK?wÚdòìCÒ?Wž'IýCr?^'Sj?ƒïpJž¿?va³µ·Ïë?ïâ"‡$ç?IÕ]#?SMái®o?7Óë˜Ó¯?dJª¥¢?EuH<hëÄ?ïÙ¤°	XÕ?fzÿߣ†?R¹Pó%d³?MrÀÁ/ø?lþ§RyPw?bÆ|—#tY?ïš'ã¼?ˆöØ]%S?OŸôŽ{?YŽ0vÁ°–?‡"r[‹BÉ?‡ÑìEêÄ?ïF'‰±Å
?Š¯}ï_—í?e«¥È?Œ?pI"Å]c?"…š
0V?‡¾7›"=?ï©æônI?hxcú(?j†ÙöCz;?U€ö¼]´~?}ɒµ¢e?d…xo¾WAGN4FGL J1301.6+4056¿Òq¤¡+@Siì,äeÀ;*@tdVÀ<Ö=Jä*@ &H½´"?ý
‡¶B?Èr_™ãA?½N䔔¢?õ")'°I	@µáL‹žÚ?¸f§>r×c?îŽCû"¿ÈydDùb¿áR"!7]9¿æ½+o"O?±Ô¼ZcαAGNbllRX J1301.7+4056?ïéÌÎ`†å?VÙiß0î[?3¤݀ô?#د1¬•?c¾®á³Cy?U'Ç¢@ß%?ïØíÿ™Ë?s"FÉ?FX÷A¨¨?REí`ÈB&?p½á*ßs	?ooï.%9?ï leÈ ‡?t'30;)Ÿ?VdgIÄ{ç?Zôg²v?…Y®–,²?rÎé¥}*?ï"N÷3þŠ?dÿçŸ= ?qÃE"'|æ?Te·zº57?'
Ÿ_'?aü'ô]?ïÐéo£Y"?m9QÃᨑ?E:•U==Î?:R5£A5o?tãõs
>í?kµQY±›?ï'oYæ6'?ŒT›_WÙz?Zýü4Q…?f•,R½Á?Œjñû\?‰Û"›gu?ïRß÷T"^?€ðï¸%s?^"rU8êÎ?[ÅÏÕ2?"ÁÙêò›¡?€LÂÍ+Ù®?îòK#¿Í¶?tѳ›^O?r`\Ɔ`?n312?˜ýk_¦W
?~sƒ¢7ÖAGN4FGL J1301.6+3336¿ÝœÏ¢Ó~@TÉØ­«ŸVÀ:z/w¼ÐÀ<t[íf H@êÑ;F}@cH9Tµd?ÏAQ'Ó?®…-âønw?æ}+Ç.'@ä-̖ñô¿çºÂ^3çä¿ã1¹€¿®¿æšýqÛ:¿èO–áXu¿ïûãp}@¿ï´ÉÀþ¸WAGNfsrq3FGL J1301.5+3333MG2 J130126+3337?ïåÔoÐÀ?›o[v
?Js16sÙB?z•6xW­?dN_a¡ôõ?"áQÅî¬Þ?ïÑE㗝?w[䭖2%?K'ÖK…7?[¼Ô€¤ü?sø+[75?s-¬¾hö¯?ïwÜ#=-?l¹(åƒP?U÷xhº³)?FL§?J*ԑ~?XÞ(ï×L?ï¾Yžp²´?_qcŸ«?iµkKO?Pé|ØY"$?søzóä°C?WÊä÷Ý7ü?ïØòK"?vøþàW?S3k•	ôï?YnPÌëe?n]W °!6?r@ÐòϪs?ïfihÏLY?žßnxA?\š¹‰3ÿç?i-¾Ç«ñ¥?'i'G'íì?ž/ìhۓ?ï(2ѹp¥?'4þ!t?bw
6†m!?`;€™Î^Ñ?˜ªÄ},Ì?'Si¯R/Ñ?ï>À¯b?€òÖFR/²?'ÝYÏ4Ÿ/?sDJÿ¢øì?rzLˀ_?wIœ)ŒƒkAGN4FGL J1302.3+6901¿ßÌG€G8@H:}ªOÊÀ:ëè&Åf§À<ʞc,ö@bdþ²M@›?{@?ÅM%ã‹"?¡ðþ…V—?ÔhöÎþÖ4@UÞÂî| ?î²k!·	í¿çM³9ä'¿è-ê¿îI
{^¿ÊϵŠeõ¿ïþ2Àœ'ÈAGNbcuTXS 1300+693?ïî‹Ì&‰­?XþÝpRX?H¶}0ÚP?IB«Ö^h?V)^¨M?R-G™c?ï¶ÌvÕc8?€1[çbGn?XqJzŒ¥?cnTÆÿ?~}r/<™?y—©]¾˜?ï){'Xê?‡‡ù¼¢Â?lN_¼W¤w?nB§!
Ä?—FÁãî/&?…7ÍþybÚ?ï鵈¸uÓ?I?S
?J'Êó|Ý?9ÛM%®¿?_Kˆ×7?Bã2É!?ïᴋŽ?pŸ£b\ùÑ?XLgÉ%@?a²è?-??b%A1;të?gêË鷏?ï;³X÷+à? ¸´T†?b¿^lu]Ë?t¹¤­p$y?–1©kD?žÍ~C>þt?îUK鞦?"õ#MÏü?'I.€x5?'–ùô?¦߶äw?'rïÓæ[9?﮹8<Ô¿?n •_9d?hކ>»*"?a¬#Ù©Í?|4 ±	ÿ†?fîX¨ÚŸ‰AGN4FGL J1302.7+4750¿Ë™]‹Ãºw@QJS5À:ûâTôNÀ<¿cí@»õÊd@Xb—¤Í?Ä|`8Nû翶µ_©D?ðùV̕o@'âý:Ó»?¨gmޑª¿ìˊw½¦¿¿ç§{9\B ¿áÁCâWùf¿Û!²Ø/Ÿ¿ïÿÅbu@AGNbllTXS 1300+481?ï…<Gƒø?®Ä};¿1?\'NÅ(GV?YÒêH2ɬ?‹,7>§þ?®ÇP&­«?ï˜îÖY_å?ŠUÈæ¨?dD|úÜ?s%öÚËf¾?" &`ëû?ƒ{8ÀóÉ?îð7»á ¢?s‰T?t&҂é[Ó?v0žÇÂî?œïSàQäÏ?t#kԊ<?ïÉo2õ÷?bM½m'Œ?a‹"uÞ¹?R'5'Ô{?r'¤Ý\ùh?YoSïœ'º?ïCC¦jYÝ?ª²œÉ§?påEâˆÛç?r§¯8"ªr?"^9»oX?ªNÙdØ?îÿ~èé8? ˜"ö¾E?tª˜kÇ{?†?åhèi?šåŸýAüÓ?™ÿ‹/p)?î#¸|ãN?–Œa—J?|²¾Œ¢Ð!?yŸ{Ñt¶½?ª. oyD?–±£5*­?ï+,89¤´?‡*ÈÆüÕÞ?ƒM½°»i?{½Cïôl?óš eÒ?Rì¨1§`AGN4FGL J1302.8+5748?êîŽŠê ½@MŸ©\…<À:W8õêÓHÀ<¾r¡L%@ÐÎý'@Y?¼®q˜?´B®Ñ9C¿5¶p?I?åÃ"ÿßHÐ@sã*\J?bmˆo¿è=þ"Ci¿àöÝâžÆ)¿âEbk¯ü¿âe!«ÌL¿ïÿÒþÀùAGNbll3FGL J1302.6+5748TXS 1300+580?ï4â7¬c?ÁG™zB™á?hñ*cy¡ª?"[O"ºM?–E"ÓŸu?¿QØem?ïá¥³`ô?nʃ•…Ð?=®T‹¯?JtÛèð?k=øoÀ?jµUÖ&?ï–à"š@?…LڀþÈ?duª‡¹R?uÔg¥é?…*º\c¬?'ðZ;ü؞?ïë6Ög—?D¤6dÅÄ?P÷ó¤Ïn?4Ù!§_a?Xš`!??o'bjy¦?ï±Ö®;Öà?¨Ç‹o½Ü?_jÂG‹ûc?|n6S3?9øC#
r?¥G–ñ¸Xe?ï˜ññýçU?†®"í´± ?PϸDî‡3?YÛ;™ýÛ?‡©Œvˆö?"÷(J^ä`?ïMmãw"?Ž''Ë;€ž?h~ì"wi?smúŠB_0?"Beú1"5?ŒÄw…öä?ïÄ£	Ò36?aõcŸ¯®¿?gçJù4Ì?RMKåí?qºÕ·Ø£?\ÿŠ"-AGN4FGL J1303.0+2434¿ëy¶\·«@U–Å—Ne¿À8Ì£Ho›À;ÃÀ…–­V@u¸"Ú¾@‡5ÜZßJ?¨ÎƒKŠ©?´Ýv=I¸@¦˜5‹'@ÎØÈ-¬?Óe±ÀVò«¿Ú¡Q¿tè¿â™ÀGƒL¿âUŽU™¿æ@&Ì£¥¿ëÐøÀñwQAGNbll3FGL J1303.0+2435MG2 J130304+2434?ïàå^"
?"S"uÿ??¿Û¬Ÿií?KAµ¨×?kí"éÁ?"!?Qdý?ïÐŽ'((?sÎå­x²?JLV.¨ß©?Tìµµ­ñ?t®®
ã0ƒ?p¡ŽÁ]‡·?ï§Q?Z*e?€`Û½v‡¸?^o/0ñļ?dëšè?']ÊLF*?¦4jÆÔ?ïÙOjTT?U#';†^?O¬åòî"
?508A?nÅ\Lê?RùXF3?ïÜXÜm²>?lF‹k_ÊÃ?=ˆnfºh?5Âc³ŸÒ]?oö 
'ý2?kH½f°ì¥?ïx1—§¦ø?5\"¨?]ä¯éþf?p®Î-û³ç?Ž7F?Xòa;A:?ä÷·?"s=u:™v?g‹Óg,é?oj1¬]\ ?‰³R)!õ9?')Ÿ$ŒÁ?ï£Ii{?rë…Fë¿´?bbûŽàdÑ?Qrl»¶k4?'"ý`
ï?qBªÉf–°AGN4FGL J1303.6-4622¿ít£–6}@0s§ü2ëæÀ:±®£íÀ<AÓë¤ÿ(@¹èÁÊæ@¿@D"­Ç?¿—ç'ËÊ?Æ"ïĦ¯@ˆì9ò@fš%Ç:?ïôÁPlÕ?Ïv<È2^L¿ß—dqē¿åˆabñfà¿è×a {{¿äoØ ?¦AGNfsrq3FGL J1303.7-4619PMN J1303-4621?ï….0G¤?pìÕ/¹­i?m‡µrz?eÎÒ`Š"?p6%1ª«?b •Ø(>?ï˳ï0O?x;~o=mÓ?U¶Wç†Û&?a
:ÃMܨ?t±4ͨ?qÝËÒÖë?ïcx`õõK?†ù…Fq?u\´~$Ý«?xçX}"SW?Œs¸pW?øñ<–?ïz±ó
VÏ?g½–AqH?q/aQÿ|?Qyé—?ˆ»¼‰Q°ž?e
°e¡\?ïi%*Ïj?…«Ñ+`"?†£~…þ"?€>Û>sèä?~&~¼@?r vÍz¾?ïnӇH€š?'g¥³n?f'˾'!?sØ+¾µ]ö?Žª–;ø?ŒÐ§DkÚ?îä'S+öÿ?'0`þš»?ˆ›Ø R?…GCÎp?—eg°4Ýû?‰Œóë`ÿ?«><?†DÞ3žÙ?…Óïo©?lh–õr?¡o]šŠ¼N?"xí°|ÊAGN4FGL J1304.0-5539¿ïÿ%¾;˙@´Ì?ß À9ésÉ%x`À;‹)ƒ‡@äŒu™µ@1;â.^?¼a™¢þÈ¿§ïС²[¡?ç2t[òo@›yòŠKž¿¼Ÿa.Ä
¶¿ãk›ŸXJo¿ëÐOt…
¿ÝC =͕õ¿ïþ"þ?ïâ
;Qå¦AGNbcu3FGL J1304.3-5535PMN J1303-5540?誩
óŒ?À	A	rV?‡Ò''˜?ƒ`ivš?ËØ2±ƒQ?¿»l×]Ž??ìW]Mt?»y£"ÿٕ?ljPœ Ã?…žCÙeæ?½Çºƒÿ?¹È:Vh•?êpY¨N$?ªp$Á…Ú?›hŸ=×ØÃ?'ËMãçV?ÂÒê±lҚ?§ìñ"›?îr¿¡ž©?ŠZ)vƒÛe?m½—Ñž'Û?U¢;Ö§5s?¦úJ†ÒeÀ?‰3`Ny?ä¸0ç?Ç.ð´ùÙ?¡"RÖ
S«?˜À$"1W?՝H4ø^?Æÿøí«ÙQ?çxΆ=úÀ?Ê«¼`1Ý·?ŽlSI™?›‰JþN˜?Ðþø²È"?ɐSŠ@¶)?äø"Ÿ<ya?±þ§GN•‡?®¥g}ô•?žÍ»—í³?ÒKÂ{ÑÌ?°o—`†?êÕfŠ§¨?¨tA
G"?=·&º'\?}WyŒ$T?Â֌o ²ú?§Õ³´ÏŠTAGN4FGL J1304.0+3704¿ÖÉN1±@SíKƧïžÀ:ÚñfàêÀ<žÈ:£j@Á›÷—ј@;^ʐ²?ÆcÄÄ?±h^ÊKú?æ¢6Æeª@¹©ñb?ïûùá
÷¿à™Ò¤}"¿çڄßÄK¿á¦W¸M¹Ç¿ëKz‡…šß¿ïØODù"AGNbllWISE J130407.31+370908.1?ïÒbxù™'?p¬1"È?UQñ*´8?Yê½-´wx?qz`—5×?i¡Êüü2?ïÑæ³dC?tÛéV
š®?H"Žõ‰â?R½ÙüJT?süj'!?qá
]Õ?ïŒj#?€Ÿ"±u?hNQ|¶h>?pñqôÆZR?†ÑæŒó`8?{óÄÚyVƒ?הּü^¶?`)sž_µs?pï™;V½?Rέ£)ü?x¶e\Çw?XrO˜æŒ?
Å´]?˜q\(ìÔ?aXk3z4à?UxTFö€ó?…úb''`?€7Ø¿f?ïqT­›?"ÖSe+?V
¸ր¸?b~€¸Èñ?tŽÈ/Y4?"(H÷Õ4?ï7ë:rF?ˆúý°Ç?kÞb‡BÙ¶?lçøddµ`?•†ÌsœÀý?‡"—<–5?ï "%?$17\B?ˆE¡gם?qªå–z.à?"YÉ&¡–?xpkÜAGN4FGL J1304.2-2412?ÖÀ¼?®8@CH×ðí=†À9Ëúú݁PÀ<(ÒO̲@÷õÄè5?þNŕ æ•?¸òƱ¿S?°­Ù'è‹?÷OÙý6÷ä?ÿA‰BŽ?ë\|m8è¿Û¸¬Cë<O¿âkb^ÄÜh¿Ø6%€íü¿àk'³ò
t¿á¶}euüAGNbll3FGL J1304.2-2411PMN J1304-2412?ï²³=|Ô?n›ü<Rsò?Wכ"Š?Fœ‡çW8w?€X=5¹?kØâw^|Q?ïoX1¼²ñ?‡Ã¢XdX
?o¼%sK¸û?rhª}à]%?Œ:ê8wӒ?2Œ†îì'?ïA{=
&¯?ºß"'«X?tûۓœ"?u^@hØ?''¡}"©–?{‹Â|Kü?í9"çªõ?ƒêêÃýv0?šgÀd…?s LGv?¯9ÿw'Sq?Z#Ñ9?ïiž"'&?|µŠ=ÁŽ¤?l'†ª|‰t?Zaø6=ÄÔ?ŽsÚ5?xãYü'²¼?î_œàBlÙ? +£†}?"Տ'û…?ˆyÕ
Æ?¤ÐǍ?˜–.Cùî³?î¹E€Š w?Ž™º?{#¤ä•/@?r\<÷?¡3Yx&?Š¦	ã…?é_:F€v?š.8 Ñ€?®'ñe¥¤©?‹1¦ó«?Âß¾X{þ?—-¶eùHAGN4FGL J1304.3-4353¿éY¾/ٕ@2êœo6ðÀ8zËïW;PÀ;wg)ÚÄÝ@E3'¹XQ?ûÎU}àÖo?¥Ø‰n~7é?¸Lݾ·‹G@ÅO±@|÷xÇçá?ïéXÎG ¿àùoߌ¿Õf¸Ü*ï¿Ú
ƒ÷ÿ¿àƒákÀB{¿Ý_ò.+AGNbll3FGL J1304.3-43531RXS J130421.2-435308?ï쫌,Àö?~eG-ï-?@e펀?T¸(w+ÔD?^œ´wߔ4?ylæq‡Vt?ïΓ´'ds?t¨¨•‰äK?SàPýécR?aô6ð?s¾¦¤!»?næÔ?Qþƒ?‡!÷I?mzûÎ1ñ©?yÜxÁ#͘?‡2¬|T¢4?'R¿Sî?ï3¡B/z?}@óçÎì?d¦ÑH±‡?H9"R"'ý?±­œã?|AÃÙ
D?ïê¸Úk_¹?W›ïZÈF?:JF÷õE?3-\"€;a?aýÜïěh?U»|¯?ïvœ²†X'?'vXxp?h7£_,ï?|€Æœ®L?ŒK­S?ŠsZ±žá?ïWbá\âë?IŽ-CžÕ?wUÛ¾RÀ?ól>R?Ž|Y×\©Á?ˆåõˆoà?íÍ5aF?–-˜™³R¥?t¤G¨V'?`Vìºï¥Î?°M¥b@5&?•ógirAGN4FGL J1304.6-0348?»žjÜ—#@MrK èBtÀ;g€t.¦À<¥Ó`dĦ@?d3?ýùÓ`dĦ?×@.C_PH?ß× ìt2?ýŽ0"óA¬@	/^Ä;¿é«æ¾š¨¿ìì©@։å?ýz¿ŽËµ¿æI;þ]éj¿äþø™q¥¿ïÿYFÃ2ðAGNfsrq3FGL J1304.8-0338PKS 1302-035?ïËkfˆþŸ?yâSè6?K†D†œ¦ß?A{K]F8?vل1"ÅÑ?wåÍ*ú?ï–h'ÂÍ×?‰Æ¡ę?d
'+×À?qåØ5-'É?…b•˜ÐhZ?ƒ—¬¡_"ë?îéÃ(ß?'a¹ã£ï?uC×Í\@Õ?v}ìïöÖ2?Ž±Ÿy÷K?'Ô¤½6?ïA]'•?s½VK1õÐ?bþ=KO¶?GªÌ3*?•Ô—ôa?r݂è(N"?ïZxG]?'Y'cœ1¤?cI7¢ÊÂ÷?[ç&J§?'GÐ&³ü?'¼SiÛ/?î×­jJ»T?£Bä2tÿ?tê'OÉí?'Æb€Jä?ŸÏÈïaf? àw•áô¿?íá-3Є?¡Aé¼>+¬? éx`Û(?'ܛºò?­ù£pŽÝ? K÷ã?íܤ£¸×M?"—U®'?o'G0«Åq?`Ú1ixw?°ȨÉäð?"/[ØßNAGN4FGL J1304.9-2107?ç™çÕR@Dл¡+^SÀ:bßÔçM'À<>-o|@š,œì	~@2ç-¡"û?Ä_DB™®?µÏžcWé ?ï'ø!dS½?õ¿Ý5¥©?î.Iq?栚tŠìX¿æ:)Çy§¿ã"9°ûµî¿à‡Ý~›<¿ïûï< AGNbcu3FGL J1304.9-2109PKS B1302-208?îó‡d»8?'ê5¼›|?rz'=:æ3?|ÜxJ™H<?œðzÂbw?H—=íê?î×%€Ãÿ?›ÿƸˆ3?Šº
aߗJ?˜ºo©»c?—¾J¯Ï܏?)PË
sË?î÷혰w?fòçäa[?`»ù‹1Ð?~Œ|áa3>?™DÓG#û¿?‡=Á»¼¯?ë1†øN¨&?˜m»Å=ŒS?±Wø¼?"\	¸‡èº?´ÖªçIЯ?Ž9%vÃ<?íã/j%ã"?Ÿku—.?Ÿ³m
Œ?‡°-¥ú?­e…äßR?œ¨Ûš´»x?ìVü¤çç—?¶§z2'%?¥M6ùÓ¼?­¨bqO¨©?²¡×{§k?¨(€€,°ï?í¾B ¹s?š¹ÁR&Z¶?'6–r¦CT?:²à:Þ?«€Š¹]Øn?"Ÿ˜Væ{?åù«ßä£û?©±ÏgÔ?Á^¥qíX?§ AWÒé‹?ƺ«nû'º?¢fÔ0ª}ÿAGN4FGL J1305.3+5118¿Â5•iš^¢@PkM:'£À:îòüÀ<Å'o(­@1æ×æ@;Ù_'F—?Òü4g??Ý_+ÿ¸1Š?úY
wt¬@ò!°~ã`¿ïûUá³äž?ïcóÅ_¿ìoC"º"¿ê§Š$Ô¿á¤jB"ùG¿ïÿ³ÿÌS€AGNnlsy1IERS B1303+515?ïȗÔ*?u/Î&Kì?pՃJìŠ?nªý"4È1?e½Ût-Ä÷?he::83?ïu	–E–?•ÍÆ?tÛ<|âŸ?'šð½¬n?ˆM_Å!-?Šsf}X2?pIWý?•WÚìÑù'?'~̙@?‰¡±Jx9Ç?žìr™'D?ŽÃá (Úä?ïjŠ[tV$?tTè=*RÆ?†ïþÀ
'?qF©Ir_M?|ÚÖWXÊ?_ÿ¢fä'î?菱÷GŽ?ƒ–6þ³ë?€"4Óîh?£rj"S?hÓ`ߪ?e>îüE}?î€mêzmë?­ï	ºHN?‹ÅÃ7/"­?ž*•G'ñ\?¡°‹i#\?¡g!`¯Ù?íÕÓb¬â;?œ:D‡^ý"?–m'è
Õ?ä­CcÄ?§l6Sï?–zk¡¦½Ë?b?– (ÁÑ?¢­=zÞ#?'û†±{Ü?—s°O3\?'xnòîAGN4FGL J1305.6+7853¿ì©Q§´Ü¸@CÿyÈCÀ:EFmCÐÀ<¯:ঞ@Œè0Uˆ@ðàpÀ?¸­G`ç¡d¿I]ÏÖüØW?¢Èè!ù
T@­˜¤§Ö?ï]=Þ1ùø¿â²ªפ—¿ä'›…,$K¿à;ú'½˜¿ç»üšð±®¿ãÑqw; ÀAGNbll3FGL J1305.5+7854S5 1304+79?ïØOÆM?d8¬•?Tk¯N€L\?D‹,‹¹?¹?mzb'*¦ô?`íõëÄԚ?ï©dp?~ôÿÐÁL?^D'VÞKä?c•Åí-Š?ðԲ؞?x§í'
·å?ïXÓ˪Ê?€o×ÖLœ¡?m'0F3?mõ´EÄË?'M¤|
bf?{HÁíM.]?ïT*:ÕØ©?pøæSW%6?…rá-ˆÍ?e™1fÒ??…'B˜J?fS|cY¿Û?ï©ÛΝ\r?xžö¾qx?jfØU±Ø>?`¥:¿?}Þ¬–öúç?sw"U(Ê?ïEAä¸?—I
/Ökä?qbzšb-Ó?wÔ")ì$»?šž¹¡'?"&(¤2%¡?î®N¤þ§?Q46N¬È?{Ó $ôé8?vIÂMŽDy?¡ ¡¨_CØ?‹>¦ z½?îƼùG?Ž"5x̉?žï¬[çR?Õ"à.¾V?žx´sïÏ?"϶˜I†AGN4FGL J1305.9+3858¿í=s,aK¹@Sq€ˆP›úÀ;"Á¯bX»À<ópˆÿ£@™¶¯T@·
è`Ý?ÍSÄ[d*?³G`ÖsY?å)¦¢@²"@ÖAj®u?ïúÀ~gå¿è™K`P¢°¿Ò¦…eZ!ß¿è17æ Zé¿ì;yÞhUª?âɛ?-±AGNbll2MASS J13053124+3855218?îýÇ'`0?™å°9pJ?h¾òð~&ÿ?b`?/<¸Õås?˜¨†'ÿ'?ï\á˜ivo?'k‰ô‡'5?m˜Ü ¥ž?uìÚøISa?°±v»?âW4?î(r1‹O?›8șBxú?'ÿÞҍ?'½Ù–"Ž?¨¸æùº9Ï?š–@Šé?ïƒP?f%?m\2µò?l¸s--Ž?TÐ_b•é?‡ýÓJ­\Ì?k€(÷}?ííðÖ9?±5£¹Ï ?{­M;)DE?sœÄm—?µ £¼Íö?°§äËq-?(ƒNK?¬"y¨~p?sóÎÊ?ftÍãh?¤†iÚêÜ?ªïù¹Ê#–?ì%kkLÃí?®uLˆt?‰°05²&t?…³Ï([cµ?»žžž´Í?­ìEÞ½'?îQ"€¥×À?~+l#ñu?´¿Ý̉'?s,¤Ã­5 ?¦y—úëÀ™?Ž^*$U.AGN4FGL J1306.3+1113¿Øc­xb@RmÛ"Ðå`À;1Óºý—À<£Êz5˜@ }¹!]¹?ÿÀëíúCþ?ÅџÅW¸y¿l‹.|'3o?¤ëÜ1™«@Jc]¿ïÿý±q&´?ïÿáÍì¿Ý ÎâP¿àÅ%ƺd¿ïïícEI¶?ïYà37AGNrdgTXS 1303+114?ïV¥Q¼?›•{‹³†?dTTp8¯ñ?b'A£YÓ?'³sºý~?šg"âöYä?ï»y7pÑò?€£†xnÂ|?XÒïõEË?nɛ#æD?|¨S4Ÿ3?v¸ÁkR?퀪Påºs?¡# Ï0
ì?'M"¿a•¡?Ž]o@€k?¯N'c)ö?Ÿ¬AIÈâ7?ïK®±±Ö?tÿÌÍzQ?yòù^\ û?cÝY%¹ž?
k
ÿ?rùÂ]¹î?ï6Xjû!?™|y3Ð?säv"ˆ@?rÕ»ør€?"3T›VÀÔ?—¨ÕoàB?ïKéπË?•àjØ?fŸdQhÉ\?ws"¬fF¤?"®ÙHª?'`"=¯Ðø?ì×÷u—Ü«?£_b<ëU¿?'_Ã™;\?šEKúå?´¨SŽÐñR?¡Ï‰¸Ó¼?íþÛ±
¡?"<èÇÁá?wð6YÛ?"µ‡'¯:X?§âš*Ã`?ékR¯0wAGN4FGL J1306.7-2148?ï1¤"'.Ê@DuöM½ùÀ9ó~°à<À<,YÜë(@s{ϯ*P?ÿ³!Dô%×?ÂGFe•5?ÉL²`9ü{@¶n¡žJÙ@ ZÑ1áO?ïþá77¥¿çšf³"?ã¿Ðƒp!ûþ>¿á†UºF¸K¿éi¿·:"Q¿á^˂Iñ¼AGNrdg3FGL J1306.8-2146PKS 1304-215?îð¥¤6M?—®ñ"J5a?‡ÚžÚf·q?‡&gDs&²?•ýürž4?ŽïÈM¬É1?îÅ×ÈJÔ?›ŽR
Ÿíõ?‰3u»R'Ø?‰~µ×V­P?šÅÊ)Md?"ˆu¥"?î9T‹{?š¹Áe4œ?—Ä/oYT/?"07}Ñæ? "òýêÐ9?Žåjú
š?ìà…QŸ@?‹Ë"²aä?¢V˜u§¤?~%Å(j	»?¯©?È^?ƒYhXiz?ìôÂj{Òg?ªØõO¦?¤U4Ko3?›åÏ°µrœ?¬^¥º[?¡Ò	…ai­?í
žÈ
Mê?®|Ïyôdv?›˜;|%? ™ϬT?°ÄúàGF?¥"ý`t|?뎜Â\Ë!?«"J êÄ?°†±òlHÇ?£í(d‡šè?³gùcƒ³?Ÿ6øƒ—¡2?èàî¥Ã&9? ‰é]³+¿?³=KÍÏO?"Q1uîę?Âú¦ÂՅ·?švOÌøÀAGN4FGL J1307.6-4259¿Ìºð÷ys´@3ÇÅ£ãŸÀ8¦17°pvÀ;¼-Qqâ›@Y24…˜±?þvbBw†?¤­r¿e00?žN%ûÎ?ö˜l¨ŸÆÚ@	É~8À¿ØàᬭȿÍc)Å÷¿Þ$_۲ĿܯD3‹ž¿àÛçQ³Pû¿ÔcÛÝrAGNbll3FGL J1307.6-43001RXS J130737.8-425940?ïáNœ*?cL›÷.U—?9"ÐÝ¿c?1#5l"ý?kŽú¬sƒã?açÄEyçº?ï¿Ñöœè?zôÚHe"e?Z[U ¢J¹?fHHÄ?y€/`xå<?sÕ,²Ý'¾?ï{yá ÷å?ˆ[°wN ?atuS©t?n¯â:X$´?ŒÄ">?†yE¥Ìcä?ïª"l«>?xò"LØ«?xÅk$åµ?Z¡#¢+Äk?™vÙ6×?t¿[R²?ïÁbõž?uÀ/ü	4ä?Kq!ý{³í?COnÞ§îã?{à;ïDz?t€þå3+?ïWîéN°	?"x[­ç¬?hoèúa¦Õ?t"ï(wY‡?'ô%½e?Ú¸÷1?ï7矮S?ÛCnOû?h·i?Š´?sç–—#¥?•ì߄®}?ŒÅÄðŒ?íÒ)®'½h?'‹'̤;'?‹N÷CtÈ?qp\-°@ë?¬	§H®Å{?)©"¡á)AGN4FGL J1308.4-6706¿ï©LÎÿpÓÀ*"'AÀ9!'ˆŸÀ;™)†âñ@ J5Ù*Ô@½¾hê?´uÞÝp‰?¹YÝìÚ´A@ÿ}>@C@ké?Ÿ'?îçuû.ßç¿ÓЕ"60¿ä¬j¹¦¿æ:"`R%<¿äXÞ=¿ïÿÿ" 5•AGNbcu3FGL J1308.1-6707PKS 1304-668?ïvœ‹ULý?­¹PFGã?oäûô(ðˆ?­ìÈz3¡
?Š_ž:y?zRQ¬o[?îXÔââì?²-'ûPàò?D°› Œèñ?Tn!´ÆFÒ?ªït¨8?²½š¿YS?î"i¢—*e?"c]hMã?{§&Åp?}	ôm¡(d?¤Dƒ×TT?'º#uý'z?ï
5&í?lGû])4?[f†ܾ?@V¹BðC§?Œ^p£¬ ?kkô†)?ï$I³¨8™?^¬µ_…½?Lá"0ö>?b/ߐ!·g?š½mv_Š?rthg?ë@O0ÈRr?¿"­áûH?Yƒg¹ê?nÌt5
?Â˼n'Gd?¿oºQcä›?í§þÂY?Ÿ)x©œâ?†³çÕet?†ü5.ÛÁ¤?¯âIÒ*0Š?›òš/ÏM?î‹~•K?‰J\jp(Š?uƒÊ"lN?^â%FF?¤—k
e	?ˆ¸±´XèAGN4FGL J1308.5+3547?è©+'ԍê@T&»ó¡MÀ9ëÂÐʈOÀ<f½Ž©|@j°†5á@tÌ?ß ?µóÁI5ÿ?Í[‰ûkò@¯ÿCAž@Z3k	?ïnÙgÒ¿ÚÊZ+ŀ¨¿ã¼œ2Ñ
¤¿çGÏ[¦¿ëä¡ÿ¿ïÑ ;tJAGNfsrq3FGL J1308.7+35455C 12.291?îÃðáÉ&?°Òãê°'?›Ö'æz‡€?®õžú¾?‡V¡à*›·?'HÂNŠÖ?ï¸ûZe…?€ûÀûê8ò?]†'A5?gì&Úq?|;L<Å1?{FY5½Zv?ìÇÅԋ0?¦¡…euŸ?¯ùùŸ¡m? å"Ԑ†?£‰©öQú?˜ߕˆZ0?ïµ¥«ö"p?boO¶ÿ–?tÏmç":n?Zx)xÅ?p]¼,ñA£?S;{YO@?î<0
þŠ#?¡®èʐO?¢H‡å.q?™.ñÄ£¿€?"Ym7C–¶?ƒ=ë%°ò?ï<Q%Ñ9³?žÒtAöd?p)ÃK°^Ø?}'B¢^º?"kjpÜíô?›´Ø
‡M?êϔ}P
?°DBà¦?¾ ˆÝx…?©×i´©´R?±	pÓ8?¢Ž²p6;)?ï-A"Î?'Oۋ‡­;?h_6‡«¤?za{»¥AŸ?‡G@Ýõüâ?r1ᙉØAGN4FGL J1309.4+4305¿Ôù!†"áH@RhVWûi˜À8êé—îâÀ;ʟGX"&@ðÀΑÈë?üMJ†6‡?§xæàcr?µb»¶úÓp@_$•á~5@aÁŸÈê?ïêv–_Rv¿ØHŒ¡8ŸY¿×4B<e‹ö¿Û}»ÂŽZv¿âÖùvy!¿âçrj€§ZAGNbll3FGL J1309.3+4304B3 1307+433?ïì7œà‡%?VU'7qZ?CﹺiÜ9?;åֈ;é?]˜èæQ6ã?Rœ=?ï‹`X&Ôø?ŠÏMv#Ÿ?i³yn­:?swéüµ?†»)"×p?ƒðW+6ß?ï¯Õ'0½Ú?wk±özú¬?f];¯8Ø?oœzz¿–³?|æÎáèþ]?pê	LÑ?î8«xqßI?†y	üå?ŽÅ)‹Þÿ?në—Xmʟ?¤ÃþŽ´?'è`¿ƒ?ïÒdžq/?ncò¤…©?RgÁL"lÚ?O:ÍòÝ37?r‡N%mq?iß,¥—U$?î™nçqò>?¨‰IÿÎ8?'êRÿ·G?Ð±ÛE:¼?¡ãñK@Í?¥A>¦¾L*?ï˜dŠe–?€¼µ&4Á'?j@'höÍË?rrCC•ŽÅ?ƒVӖ«€´?ydÀ.Ú?ìH;™šV"?°_¦%:™?E'Îç^g?"ùE‡´ð?¶lÙ?ssÅ?ž
šÙdÕAGN4FGL J1309.6+3718¿îwÅ~@SÇiÂ;ySÀ;¿B$g¾UÀ<õ²6ci@!Cš
,Õ?ýåù×ÇÓ?ÅxÀƄ3V¿¨ŽïÇx¥?äòÂàdÚ?üê#!BE?ð?àØ ÀaŠ¿ÃSGOÊÄ¿çñ-Õ%`ã¿á…\–$?Ä?ՂþÍ{AGNbcuFIRST J130948.8+371651?ï‰ùÁ«??œ¤ š.??*}3×õú?FéSR¡?Œˆ;¹™³(?œbÞ5n»Ž?ïA}ù!‹ã?šAÙ¯­Y?rÖ
"óT'?|¼"â®b‹?"½y%co?•€Õ-D¢?í—ú{ÂÕ8? QS!îšÛ?pÖþr?ò6?sûC¼"Ï?²2¼;(KÙ? KëfÅû°?îd;JÑ+ù?Ž˜mâ–¦?‡ÿÁ†çs?tI=e+ø?£¼"÷я?ŽПۡ(?îƒÂøì?¬zì*™?N¹ê§ñ?Rx|±Ù?§Hì@Ñ›?¬:«C´?îA´w¸Àž?±È¥Óg/_?Xîv?˜Ï"
¹…?§"bƒ`zÈ?®­¿~K?ì"x:ßò?¤×Ö×ýí?uá«"ý^Ò?vìxµÝ•Ç?º~%Ešúÿ?¤‰CCÂ:?êà,S×(×?«¢Jª3Ÿß?_†enˎ?•‡Ü¥)g?ÀÓ]⫨²?ª'èI¢WÑAGN4FGL J1309.7+1153?ä­ýJ²Å~@R‹">iƒÀ9ÉQì[ÞMÀ<J@~uPå@-Øjå§@%ð|Õ=µ?µ ÏXmTl?¯S"'Û9?÷–…³2ÇÓ?ÿÄ¢–?è*·c®ü¿¬À=àÇg¿ãshãh­¿á'­Ãó	¿ç¥¹Þ²§¿ên¹PïÝAGNbll3FGL J1309.5+11544C +12.46?ï ,,­O?qjkÍÆÙ?_býX4dV?QKs|<§?"•>Wáä?nÝwŠ"%é?îÄø(Vq?¤-
‡êÛÜ?å¦¨ïϑ?™ZsÔá4?˜n' ¹æš?•¤ˆ€¯¢K?îÿÛÜ£ô*?Œä±i?ƒ0"Èw?'›NFRSn?–l€'^"?"Èe5Ä?츍y"…L?"N'ƒ£D0?±‰jrÙt?õÏnw…?¡e!'ÑøP?{"â™"px?ïØV)¯?ŠÇ§M¦?uu¿'ˆò2?qñ«íÆÏØ?–§…\Ï"?‡8ú¸çif?ì¼bH–ê	?µ[
–®ä?¡XƒÈΚÀ?§¿êU袓?±p«×½IU?¬§ä•ST?î&^S??—:}x}tˆ?ŽÑ명?ˆÿ—C`Ïd?¥ë3ϗ*Ê?'k#;MÆÎ?è½/ãié ?§Gí3†©?Ãnß¼h¦ˆ?¥Ã[…õZ?³8ÁiK°ô?'Ûֈ•îÈAGN4FGL J1310.2-1158¿æ/š½¹'@IPØ]ú‡À:KÏknÀ<UBí»YÞ@ˆ_X@$(ƒ¬ÈK?¶þ"n\T?'¦Ø؄ø?Ýô^´kW?þ&'Ë¢¿ï(,ÚSž
?åzVs'¿âœ°ožôL¿ãdT"—½¿Þ¤‰ôaf¿Ó°
ĎºÃAGNbll3FGL J1310.2-1159TXS 1307-117?ï¥ÅMýd?{òÂE°qv?^šzq""?T\!'4h?'æM ú{?xyó&¡×
?ïµGӆØÕ?}9ȯKÿ}?ZÍ=‹ªÜK?c€Áè?~¨Æè:3?u¹Þ¢Q?ïDþ¹Ñ>ï?ƒoÓj}NÄ?r¥©œ?ìø?sá÷õ!,.?'¶¾XðÐñ?€çÑ$ë0?î×O¼?y‡h®?‡ˆ'NI?i	OmMß?™"¢¾[p?sÈ^^s=?ïHOhY@õ?Š_ü6i@?qmåÌþ?d5=ʞô?'µ·v=7Þ?‡=í3e+U?ï
àOØ4?ž  LzÒ»?qaŒõ·Ëµ?|Ao¤d6(?šK'܃Q˜?šDµó‰¨t?ߧ?'oK<ih?}k72P?|Ü¿v?¡0°:¬¿?zŠäÎg?í9½ûM¿?"@cX¦˜?š¥ID$n¶?"º.ôæð…?¯_Óº?)0a,üÉAGN4FGL J1310.5+3221¿äô  ã@TÕ=1¹¶pÀ8M_ŠªŽÀ;[ß-ø`Ï@³±_^	v@eÊål?¤6NàQ¨®?«DTÚ<L@`ù£v'@LVjoàc?ï%tc+Y¿ãE& RÆK¿äe·]®1¿äF'ÌÍ£Œ¿ç™!ú{²¿éécÜHkAGNfsrq3FGL J1310.6+3222OP 313?ïöõjÙE_?Ds¦|zçD?6¢K?¯?)œC&³Á?HÙ/‡I©¾?A&¾.MöÙ?ïËʬ6??wIܾĎ?L''ºMŒ?U?…ÃÐ,?vˆYžãu¨?súLšáåÝ?ï
Ôö£4?"S'@M?âý¤O¼ì?…`ÏþÿJ?–¬¡ÁؾM?Ý8›˜p?ï…`]ý{?wwÐUGL?p«sUt?\Dç@æ'?†R.ÆÈîõ?tÞbrM;Ó?ïìӚhÃÛ?[ƒ+ïI/é?B¯sPGùß?9Ö±øö×+?]ãƒMÍ?Wím]#è*?ï`˜c¹Ö?•Nâ&¡?_á%Nå˜?p¿/ë•?'îá/ìh?"cTÑGï?îgø*"Ê?š4R»è?†¡ŸIXÅ?ˆ-¡("@Ä?£Ø'Ø"Ô?—ü8¡çXÛ?î.§5¶E?™›''©(?'"Ç_tÁ?'ˆ…ýôx?¤*¬úL?–ÉgÆ\AGN4FGL J1310.6+2449?î3)ß]¯@UG"…]¢sÀ:Œ—f¹rÀ<'Ã}˜²@ₓî‰á@o–Aö?»¯£½ú¿¥Ù«#ýÀ?ëᣦÙô@SqîYåO¿äêê>͛)¿Üº[_L¿ÛâCV–æ¿×¼Ù¥"cØ¿ì³+ ?:¨?Öôû?&£AGNbll3FGL J1310.6+2446CRATES J131038.52+244822.1?íâLDth?º•SíEœ?‹êƒ6?•ŠºEÚ¬?ªà»Ù>Ýý?¶,…;‹æ?ïšiE=÷²?Z"µû³?cÆ
)m1?y&ûÊ?Ć?"t,'žP?†q8ÓõÐ?íG.×r±è?¤=u‹a'?—ÝÏh-r?"S'˺–#?¯¾#¥lMÁ?¡Ô‹Ñè'?ï–YR¡?{ÞMCýË:?ˆ¸1	bT^?rKš"w™€?1T4å¯?qýÌÄR?ìxM³ßbs?»¬êˆõ]?›~#ënWß?œ.ŸÎ݋E?µ^	gá$m?·!?<Ú:™?xØâb?¯ÎÇÑIåû?uR­!ºÔ?~¡ž[W?¥Oë?¯þŽº
E?ëóÈqâˆ?©ˆ›žË?Ÿ›ÚÞÕ°C?•••¸ÚÃ?¸zÅÀíZ1?¦u©Ø¡E?íc-N9@?˜{+Ø;Žù?¡naÙ Ô?}š>íìü?¨a|²ç!?Vù_yyAGN4FGL J1310.7-5553¿ã_í¨†é¶@ˆ.¢ªºSÀ9§¢KïÃÀ;m$²>¬@B;䲝@SsD›:"?ÑqÉ—ïu?Ør­™+@Q˜ÿ?æ @o¦èa¨¼¿àïG€È|¿é'5deÛ&¿å)™—Ž¿ëüXáB¥—¿î¢‰,d?":#«š'AGNbcuPMN J1310-5552?î'mÐ_v?«œÍk(?bÏ[°r?_"ðaöÃØ?®¶|+?Ï?ª|{Úú‰Š?îÅà'û•?ªþŠ.ë?hÐh™º?tô ˜Ó(?¢ ö"d6"?©ž"æg­­?éâHMæ?¯
}vÀ?§D›
؝Ë?™Ïþ-ã€'?žm²ú­u?¬ÍY¿Œ?ïÑ16?
ÞLÝÿ?S™ÑqP?8&Ýû(H´?›ì@çn??€Ä 6ôaP?ê
'¼}?½·ý¿«H?bRä›ûêŒ?\žÚhÇ4Í?ǎv"ϖ^?½'(ú—ƒ?íñgêR¢?¾€oø5†?vØÔم1?ŒF?côðM?¶膃ëœ?¼þ·ü}®?ælŽ¾@ºR?²¦Ø˜ô2`?ªñN¦U?œöìÃÓ£?ϑq]vŽä?±±2ò®y?ír.sZë‰?ž¬€[m?eؗ#ÿ(â?U|0¥wé?³¿ÇªÉγ?œŸ¡r5AGN4FGL J1310.9+5514¿åGÞ&¢'M@NÔ
9À:[FóÚWÐÀ<´Näi¡"@˜GŠ®X@ÅP^½$¹?¸ÒK¼ÁçÁ?§gƒò¾N?êwAë\ÚÌ@ý;Qå¥â¿´XÿJ£gN¿åÓLãÞaJ¿åœ³"íbo¿åöØ9¦ë¿é¥ÖÏÛ¿ïýO¶÷xrAGNfsrq3FGL J1310.7+5515TXS 1308+554?ïÕ¢î¾?e'ß¹äÓ?\-eÒL~?M)iÑC¼?lÉÖ'Ê?a9'rñsO?ïËêF°= ?tΟ&Ý~?NWMÔH^7?V`I¶Rm?v?òñ¡?qÂåË$ò?ïŽ[ЋHH?€;Þ~Ù*z?c‹aˉš5?h5Vu@í†?‡†3hë¯o?|™™¡€´?ïºÕȍ¼°?]ŒKÓ=)V?r4àfmh?T"`ãLB‡?p`;jÁjE?QԎ±äâ?>…™)?€"½H>Âç?røÆu¦½r?e"~›kŸÄ?…Zwƒ?{¥p\Ê^p?ïY\2cf?uÒËp_?c½"«ƒû?kÃb-E?'sfK…ÜÆ?‹—_¨ý'?ï×Qyß?VäEíӋ?r¡²çÑ9‰?q5vð§fo?˜¼©|lG?‰`ðOՌ?ï0HÓꉇ?|Åî¤f?‹ã;nÙ%?s²Ô6¤0?ˆ
¥[?pý¡"ÜcÍAGN4FGL J1311.0+0034?í'WüdÁ@OƒqC9:´À:&­~Rì6À<Ìóc9‹@ Þ.Iš@þM œÃ?·ó;K…w¿¢!¹€Yé?éß[zz¢@7Œnbß¿âEU	FП¿×Oê£øBF¿ã{E†S¿àîÿA"¿ÜÓÄãŸL¿ÙT—¼Ÿ®AGNbll3FGL J1311.0+0036RX J1311.1+0035?ï¿ú¶õ˜?i‹û¡û€¨?YkT'{Tf?L¾{@fùñ?y§Ï̸S9?f.{<†
?ïÈ_ZC)?uÇÄ}²ƒ,?NíÖþ™ˆ?RFÀ¶ö˜?wòÂilaD?s#ÛtØâ?ïew7¼QL?{;š;æÅ?g·ND3q)?cuÑFcщ?Z/A#E[?x˜Ò4mØd?î÷kQ»<4?wF(ÁßÆ?v»j°h4?Z¤uVÍxæ?›r¦ë° n?v›Õv–Q?ïr–#v?~—_áɪ?o•~Kô@ø?aED"'òx?‹–úØθµ?xèú]ßCD?ï`ëëG·?'"'‡ýf¨?`!¢\Îǀ?hÃ'G¶?'Þ[¯B6?ëf}Óäp?-aPí?'e­m†Í+?zŽö®ð?uU¢ø&¾?£qk6mÜ?€è0R?ìâÛçiR¡?"Töpl÷?'¥9¢óf?z´Ã,Ä:ù?´¤·w(•?"'–&-ÍTAGN4FGL J1311.0+3233¿ÔÂúªÅTÍ@TÆå6P&À9Ú J"cÀ;{Ø=CWn@®´2ø@.‡$L£?ÁÍÊùõ÷?ÐÖ\˜‡K@3Š™K–@IVå¿âÙ¿ë–ñÿ6V~¿¶ªåò7Àa¿ã,iöZe¿ã9ŠÀÏ6¿écÞAp ¿èØJCðð™AGNfsrqRX J131058.8+323335?ï°øoà/"?Y'K	t?j¿|4ÉS?sIÌp¿,?z$9Ê>æ?t¢7áÞ?ïËxõñD?|&JÞEÔ?P<j)á0?]ò9Ídúç?v4j'å)
?vÁ~³¯?ì
v5;v#?§tfª$ä?š†nû}'½?'lz҄Ù?¸ò²˜ Ñ9?¤æÁ˜û´Î?î+YB›¯?Š¤"ÍÆ«?z@ÖE"·?c"ëC(Hq?ªQ<#º?‰e†Wøƒm?ïK%—-ˆ?Ã±gû?7¯½ÊÙ?zÈVgã
ž?šÂaÚ}Ÿ?ˆwX‹Ž<d?ï`1x?–²Lÿô'Á?dU•<Š¡?s›Ãh´Õ?'qç5õ(?"x6¤©Y?é¥Î½š
?¯õ¸rƒÈ?¨…ä0ñ®f?œÔ£{‡Å8?ÃGKýô%ñ?¬ݶþ$ ?ê-Y¿ÜF?¨)ÕzžÁ?–¨ý‹O?ƒùŽ+?Äv–[òõ?§Œ"ËÊ$nAGN4FGL J1311.8+3954?ã>c|@@S"Ú<÷À;‹ì §ªÔÀ<ñ令ß@ œÜl'¡?þɋϬ{?οUÀÑÁÔ?«fÝћ¿?àóîå%‰'?ýùö{œÙ?ïý'w>$ÿ?À7`"j[¿è™â"µ.K¿Õ4¸#G'Ë¿Ö<‹Á¿¨w¿äðÖÍÏ3AGNbllFIRST J131146.0+395317?ïŽGÞ]eX?ƒˆgS´z¡?CGP
Hě?=ètÓìá?‹9"hŠÕr?ƒ>Viþ}G?ï Ç[|[#?‹¾`[1?XÒ!â´-Ú?d€+>4?"³äò©u?ˆ¡ÍUïÜØ?ïÃ3sm?ªéK~E»?k:8£dô?p»ÆQC?œ@R¢Ü…Ê?ŒL÷Ëõ3?ïUûÏR†?tŸM¦¼˜Ó?w7̐3×?`)]<‹<…?ŽåU"ÁÆ4?r™
È·‰°?îö1? ÍnH¸?R¯üvühH?MžB{sà? €åñÎ?ŸÔÙYÏ´q?ïß	²¨¬?¡S1¾ý?fDûSB(?|#½«»êÛ?š›f¬K<? ¤=@
-Â?îOoì¢?œlÀQý`?q¹€#Z?pdCÜÛ±?¬SßäÍ6º?›—j¦x5'?îÖNM7c?'©žÒ•?ŒŸÎ Â{?Œ};?¨Ê§•œ2?!Ð#2MõAGN4FGL J1311.8+2057¿Í?Ò9.†@T'(ÂzÀ:³ŒbÀ<k]Îpk@±ObhÕ×@
aûc?Åù‡€gny¿Àkí"ì±?ú
Â*²[1@"Àl—¿¼ Ì"Áé¿í66Œs¿ì£ÙŽ|/&?ºÕÊÍC?¿ïÿöùŠp?ì:G#ªÿóAGNbcuMG2 J131144+2052?ï‹ c¼À?¨¬Äø¿l?pž
Cn?'ò=G§À?…/yX?¤ÐSH=N?ïv$5®&ˆ?™Óð"AU¦?vuôǒN??8ŽSú¯Ý?‡;ø8<ZÅ?Ò+
¹¥?índ"€?£¦(?"z–ôI¥¨?…{-]?±u9ÿ/iˆ?¢@äž;%?ïÞÈUw^d?brRI Iê?bæq(Ù2?[546]Ë?^7ˆ?o¥¬?RIZ—É0p?ïD~™°b*?œæüô"Øh?"H["z>†?Šàåúð?Š—þ;jË?•ø‰/?î[—Ä6?·PG@¤ë?'Ã(µá
ã?°Ï1Æ'•f? äû|>".?§(;'i¡?ìfØ ¯QV?©xÊžÐ}?…•tz?Š'êz.Ì?¹˜ªÀºC?¨G	é]³,?ï+F€Ô?šì	á¨?'«å€à¬?™'.ùÙ?ÿ£BÌ?}eÕõzøèAGN4FGL J1312.4-2156?¶‹=á7@DUóFí$À8µÁÉc‹ÁÀ;¥'õÉE@ýêAÞG?ý:61ë5?¨ŸCãÀÀ`?Ãc>Ò£¦@Ò­`ûH@¥ŠFjr¿áËOK¿ÍÐ-hî׿۠¾øN¿Ý^{ ۑ¿å«(m"˜¿êIÈ ÈdAGNbll3FGL J1312.5-2155PKS 1309-216?ïß?Œn'?™}6‡ú?ZZÆ2qqÓ?zîBûbÛ?c"fË(A?"–	·ÑÍo?﬉XâLï?¤ƒ³îJ?\'"'Ëì¼?jx»%ü?X¹<꜍?}¯¼—ô?îÏÙ4'?š™Då+K/?—ra'yG?•>"H"¬É?VGfDMO?'9ÞP¶Y?ïxÏ®Z?r
uÕõÈ?fÞ%^$œ?PVñâÿ?Œ²¬ŸŒ¡?n¸ª_Á?ïÞñ`°+?g¤¤TA!?`<Ɗ?aYóï¿Ù?`ÒÔêbÀ?U'7¾¾…?îüº"²?§Ï«õøÑI?qò·r;"}?Ñ€Ó\ƒn?œÙÎ| ?¥S2ŒW,[?î» 'ß÷U?œï*€à?—þ¬ökØ?–¢U'G¼?CŠRۘ?3)ÿ×ù?îÆy£7±?Šn´¾Žµ?x&%Žóãé?e«œìh`? šC°Öb}?ˆZ<=qEUAGN4FGL J1312.6-1900¿ÙSQ¤7'@EÈÿ%¿­À:ê ú¶ëÀ<|K2-y¶@ …½ôAÛÃ?ÿ}"jŽ?©Â܉s?"†_ޕ·?ÅõÛĈ?ÿBX•~Í¿ë‡e_L—?ïóÜÁ6–•¿ÚÙ]ÔÇm¿áőڈw2¿ä†'ø»h?º)WgEžAGNbcuNVSS J131234-185902?ïÒ/®•ô?s"]áW×?H›†lõ¢?@÷C#ԆN?sÔ¸ð˜¥?qD¯îØØÏ?ï½ D·À?x\ÀþÀîP?TƒåA?^~0gêàŠ?|E¾*¿?r£Öˆ=ë?ïÿ·/׉?w•øŠuÑ?_nï­=?P¨aá"p?‹'Aï5BÝ?uß9*ªãÃ?îßÇîÁ"4?w÷
‡C±?|~ÖoñÔ?_HרԐ2?"pýŸý?v‹Ç%›S"?ï¶ds,?r.z)¿½?Y1ÑÇÒùÍ?NחtYþ?~°Y4àË?pL‹?ï7˜ô
ÜÛ?'¾ã¤+x<?d¤×ÓJœ/?lû:¸&'S?–xFƒ_*?ãQžƒ8Y?ïr•:1?ƒ©XÉßÎ?hvóŒŠ(—?[®¡¶ò ?™âÞ³´_ß?'t5Ý㚢?í@¦–á?'º–Í^?%'GeÆä?za *ð«?³R‰–^?'½ü•áTùAGN4FGL J1312.6+4828?ÝÙ@QÔªà"À8‹p*ÖmÀ;ÊPSÕj*@²6¡&Ö®@‡¤WÙÜ?¡HÔ|ì™?¯¾"¤9I@>vû	@ R3€5¿µùN`
VÆ¿ÜÆày§â¿ã%p'Iü¿áW^‹¦'¿æàTÔmªþ¿ß—ô}ë¾*AGNbcu3FGL J1312.7+4828GB 1310+487?ïø.‡Ê?>&Pì`Å?2ŠtMæ?0m ¦ì‹'?FŠ£iÔEI?6܍ه?ïÝûÞ)¸Ø?oœk¥OcJ??þx‡éÅÒ?IÈ*ïÌdö?nRÙ{‡?kþf
=¡?ï­X «Ó?~$~#a?[½þ˜>Ø/?`âÒ7çÃ3?2þÇU?}
¼l/«?ïÿQ‡D?ðð.&Àc>àËÔZp{'>ÒV"*w?Š?µ£¡øý?ؤ£¦Ý/?ïóýúR}7?O)8Ž'(£?4ÄXBF"?4¤mÜvî?RÒôÑÈ
?KôI·t0z?ï¢
ºKÉ`?†V«Aê?Sْ}zø?jî£<Ž?…
8,)?ƒñ™¬*=0?ïW÷AÃ^?oIð×?gîÃuK?q™°˜A®?'Le´9Ù?Œûiµ~¼?ïþ‹`Æ¿B?7|—\t>ñ^ì7ö&‰>êñ‡6–t~?%€ˆ ¼?,Þڑ¦AGN4FGL J1312.8-2350?Χ(xo'€@Caÿ.Hè§À9»¤ûÍkXÀ<*b{ö@ 7™Ig¨?ûîPrß?¸ž·¥+?·í§¸Á''@eÂÒxy@Poĉy?í¾aÔU¿àR*ڟg¿Í'&]·Á¿ÞÅå"S·¿Ò‰ÎÒ`‹¿âÍ
>××AGNbll3FGL J1312.7-2349NVSS J131248-235046?ïžX»XP?‡ß‹™Â?[\Ù¦KB?XOmxkÞ?"þ6û•Á?…&ën{ó;?ï›Ú¿1a?€¾0§½ž²?c°jþ'øÚ?gu"¥ºcç?"L.Œoaz?y­)âÞ!U?ï1(ðÜn?†Epb?mIë°a?p1¾=cÊí?–1¤WP"?"7>"Àï?íxý_fÂØ?ƒÞõÉOL?‰Sµ¹e?fǔœŒ?¢?±ŠY?'²HA®:V?ïâ]O3?Œ…¶×f0?u9¥~ÜTV?kQ
ÏæA?—zYnx‡?‰!¨ŒÊ«?ï{Ôrï?—ß݃zߟ?v^!×à'?¤ævèyÜ?š8üømøG?'ŠºL¥F·?î0¬h(]l?–Yþ]šc9?zD]'à9?u÷zîS©?©¬­Ñ³?"¤ûÿ=­ù?é×vþj?.¶ªT/‹?š~´¢ÕÌ?û±Ù*Ïõ?ÅRQ=¸?4uÊÔÇdAGN4FGL J1312.8-0425?ÜúÉÐ0Î@MÜð0$À8åö1J%À;߬ÂkJ@ŽØ™´œ@¤u_þmY?¬wìÃÂ¥?Å'Øa*'P@[oŸË@hJã©K?臕ÀÇ
¿ÛAGÞeü^¿å¨ïbxñ¿ç¸Ž·«¿ç'£²ø¿ïÿK§ž?AGNfsrq3FGL J1312.8-0424PKS B1310-041?ïÔ5‰¤®ö?gQÕÙ
"g?h•öÜF»œ?`Œ2š³RY?c4°"­§?V"ì6ĕ?ïՐ³A
Œ?qŸ†'{æ?I*õG?UqàÔ~åi?rd
H ?m¼÷˜V'E?ïNÂÑ~ëÌ?'ùڏ²?~:òL"ª?"9vsÍ¥?®3ÕPœ?‰‹¨«Š{Ò?ïð`ü«Gþ?A6¡sRÈÛ?@5=j5?(€ZÒ=º?W1k…#³Á?<Ÿ?¹(n?ï¯EÌ×£Y?y5J¶nÓÔ?p*y¨Cõ³?fE8}yÅ??x2ŸêŠ…§?sÿ¹üíÿ?ïy	nh¾Z?W·Cp¨?bÖ¯ë
×8?{íÿT?øbuí¢?‰ÌæRMã_?îÅ-Ǖ*?š]L|Ôh­?"#'ü¹¤?‡)j`ÈH?HËD
Uf?–hU»²Î?ï×s?a:òlÞ¿?T®@¶Y?E²$%òê?nƒåA"?]«[ÿÒØAGN4FGL J1314.7+2348¿ÚXò‰c°B@Tò	ª£­À9;Ñ|^öÀ;åw¹u4@dçv¯Š?þV½+o"?®t*a"ð?¸ÉÏAq9~@HŸ¬R@€\óvè?ïf* ºà'¿ßhøÑî¿Ý¡¼þ£‰‡¿à˜B"пâúK '\9¿íÍ;5À¬AGNbll3FGL J1314.8+2349TXS 1312+240?ïñÉKõ?PT†'WéU?5ú-Ü_=?*b<­=?X'.Äû#x?LÁòhÆzn?ï¯ÛØáá?ƒ2îº<b?[]Qñ&Û?c|Ѓ6;?€i@a??€V
JŸ#?ï¡èSw1¡?`M1Y?jÅSˆÊ‰?t$¶§t3?€ÿ9ÍQe!?wR'5N?îÅp^Ú"m?|'5"%²O?…Óͬw–?f‹'—¯?œh
IX}^?x¸™
~ú?ïàŒ'ãRS?`:ú¿†¸ ?C…]ç<Mi?7`yEo"?j'%lÛ$p?]Sì8:j?ï"—S2ô?œ™}LÙc?qÌúX"?ƒWºgt¢L?—9Öü««£?—?çž=?ïyR­)¡î?ƒSڋdí&?r"¢¡b‹D?x4BRæü×?ˆaƒb&?}?í4Á V ?•y7â5ÿ?–ËJiü5*?ÊE‡îQO?°§ dhN7?"t>zÀä­AGN4FGL J1315.0-4236?îcÝbFF5@4O~ÃT~À:&¤/õ'À</ßÅoá@"`3F~j?ùÿJH"®?Á5Yh§m?¥$Y%¶?çoPð³[â@̪7Ìu¿ïù>Ú[V?îÉCu –
¿æMà}ٟ™¿ÖëDÜþÉ¿ÇÃdCK"8¿ÖA_›ÆðjAGNbll3FGL J1314.7-4237MS 13121-4221?ïOÌ\?'Ìdxù±Ÿ?b‹œÁmN\?'£X?S÷?"Êìhl§¨?W"¹G:Ð?ï¿ê†ýÏ?†z¸­!©?Pœgˆ/#?YâM€§?{ã—Ov›?"[åuçk?î€å?™'ö¼uÁÂ?mËøÞmôþ?p=þ¸;?¦!Ò!pI0?˜sbRyô?î'Ÿ‡Í?ƒÖ
û³Y?x.ÆÕM?a‹\y»?¤Ù
*"…?ƒ£ÈfW?î¶Á·%y?›JkRJ?nïsµkFŸ?cэÂD	z?¢¤ïºÂÇ?™êßhxô?ïM¢í³?"Íe2Ÿ@?b÷TNýF?n¤ñþÀÓÛ?"ìÔü‡°?'!±3FÜç?ízÒ¦wñ?¤pÊEpé?{3Kqñq‹?{ö_7
€?¶ô²ç?â?¤î16ÞØ?ìKBð¯Cê?Ò8RŸµ?‹EÌ ©™œ?~uª»¥¿?º=.è({}?žq7!j¸úAGN4FGL J1315.1-5333?ÈÆ&JA—¥@"HϧÆÀ8¦m¢šÊÀ;RáNd"@Ù{Üpê@‡½#â]?«AÔ&?À^GG@֜¾H'@÷¶p"è…¿Ñ慛
¿à†Àyt¿åUD€ª³¿æ(°B¨q#¿éh‹¬"q¿ê_Sb'½^AGNbll3FGL J1315.1-5329PMN J1315-5334?ïNÄ‹jN?"}X t?_V«¢Î~*?Tžìü*{?"2ðÊ7Y?ƒç"4ŠÒ©?ïÃpÈj—?…pïû4ô?Fh%v¹Ï?]~€?{z—¦ý‡?"=ßü´¯?ïlªºËØ?"L¹…?ho9E\Z¾?k¬S®¡?Ž¹'ûÄó??ûÐËæo?ïÁ½àåÎ?]¦Y˜ø?EÖ®á—9Ü?,âÅ3z?|f:`ßñ?[ҟ"AU_?îC[.
?—üUÂO?pDµé'Ê'?f¦G[ïùý?©ÅÀoðsˆ?—=¤?(Κ?ïm*¾x(ä?˜TÏú¤'s?Z†ÕYNS?l…غs[P?²F¦¼ô'?—^Úz>5?ï8‹®ßZ?qíÇÝéo?uÊèM\+[?zûhA	?"{å°qÂþ?Œ•Õ Î¾?ïa•¢ÑË?zÐMíoï?]D‹ÜRââ?IRl$ A`?'ùýä±k?y…¸4"vAGN4FGL J1315.4+8453¿ï772W|O@@?·¥ôÀ:ØÙ.IÀ<jÑâ¶C@xIéW@"}€^_1?Æ:azÄAc¿ŸÜŠľ?׳Ûåž@–ŠýtŠk¿×V^?&¿ëpBRŠçO¿â©å‡ó¿çÁ½ªE
¿ïÕ@%Nn¿í€MÍé,AGNbcu6C B132240+850531?ïŹLMr?oö"Äê<Œ?X°œ*C¦˜?N)óߓé?v÷2åz)§?kuœ4Œ£4?ï§U'¥.?€Y#"Óî?_$ñØÉ%?c
ì:Kæ?'F uýò?yŸ¸+§æö?ï0üa:?†Û²oˆ¶ä?tó"|;?tãÖdâ>	?"öƒ™@òþ?'ëu–Dy{?ï{äyÅF?j‰Bvs?m´B(ÏÆ?SûnH!Ÿ¿?‰ßYÊÕ.y?grݑ?ïI?›Â¶?‰±2Ë*÷€?q'.pÉí?fÆ{¡MÅ?'s"¸"‹·?‡3ïdµ?ïÆ|Ú#Ö?šß¯"?ob,"".8?}Û
ÈÈì?šêÚ,pq?–.'u81?îF¸>Üoé?"âpM ?4'¦1â¹?ŽðØÞ£?§GW¦†ÇB?'¨bÁ2":?îby¸0f-?Œu…~‰¼»?† B±#¦?t¡ŽKÚä[?¤Vœi¹ŸL?ˆÏÍj=AGN4FGL J1315.5+1135¿ëKê¼C_@R]­BÃÉïÀ:" Rñ?À<eïÎY"Ç@ îRî'?øú™ú©v?É#–=áã?ËÐá.ƒ¡
@7°pu³á@Ôüj?ï)³ʅu¿í¹´V´A¼?Ì´ÆÆ£gú¿¿›Gn©€í¿×{°&äp¿äÎK^˜AGNbll3FGL J1315.4+11301RXS J131531.9+113327?ï̚Þú2?œ]|:–²g?`Q¡TnWO?UÝŸ¶«?œ\8y¾éÒ?›§rjîšÚ?ï¾7]z7?{™ÍŠÑ™?P[€ƒ«|Ê?U$	†#ã?|͛J-É?xÌqßsŸ?îóunÊ#?‹Ú.GU?c0•ZUó?W z4שœ?Ÿ/&Ôá?L)?‹?îTÛìqÐ?…Í–ð`?s(«™Åe?YúܽÎ2?¨M>ß$Bs?…=ÜoÝ&š?í¦…VoE?°Ñê¯;
{?p[Á€îù?e­	«wU?±Æ|H?°~8®&k?ïFÑo7µ?">ÀHôªP?bžWÂRV)?oÓb"VÖÄ?"ëZÚÖ —?'Ýf¢÷;`?í'ZL@+? 'DY¸?sþ@¾É?tc°
j®G?²­LŠw[º? †UÃ$.?ëž7ѱÀ?¡Kñ«_†ý?ƒ6£ËaÀÍ?tæ¼ã¤Ã?ÀS¶|d´?¡GD)~OAGN4FGL J1315.9-0732?é"Ûƒ7Ç0@Ki"}ŠÀ:
뱔b"À<(^Ì>1"@ƒkµ/Í"?üO9#7=?¹…cÂD¯?Á·uø®@.d²1@@mdDM6ê¿Ü$´?b@'¿Ù²ÕÎÂE¿¨ˆÕü÷7¿ã!¡ŸØx¿Ýa'nê¿ãwקò"AGNbll3FGL J1315.7-0732NVSS J131552-073301?ïçO9E"T?£S¾%Å­?3aÃÈo"Î?*–j'è•?fDŽwîùC?£Udµ‡ý?ïà+ځôÀ?l"¥И?@ÍȳûJR?IE¢‡©ns?k ³jVZ2?hdWHn?ï¼-à¸çé?q玛Ãþ8?X«@Rí?b7 ©³¹?{¾?©(ÑÝ?n6ÓMàÛ?ï½­[ÝT?]¥ø=çÑ?D@*$ðϙ?,	Ÿž½Ü?~¡L´ð'g?\=QY5é­?ïò5€P®?MÚ=.õ?IÞý¥ìÉ?Aւ¤X˜ß?MK¤`$È?@íDôÝ»Û?ï"w9ƒ•‡?ÿ}#AM¨?QH#Rfˆ?Zgh¬(Gá?ˆ¹->ĺC?ŒYŠSd¥?1÷–?€KæÛ7ê?ctVP[—?h< û#ց?ˆz䫤Œ?}‡ëØfð
?ïe}ÏòÆ?x0²†µ?RÝ×ã^*?C–-Jt´t?'"h–´U?wt/NêüAGN4FGL J1315.9-6349c¿ãì:¾l⬿ña၏·™À9ªl…dXoÀ:²/€ KÐ@'±…"@šTÅT2‡?Ò§9)í9T?ºM6iž2?äkž´‹g@T,Ž~]~¿ïüœž0Ø?îï7œ¿âöÙÑ.[¿â©‡¸Æ…‹¿éUDÀyWZ¿ïðdìé¢ÆAGNbcuPMN J1315-63540?ÕeÍ͆cº?Ã6Êïtc÷?™Å–×Û9E?"ªè'ó^¼?ä~ìbÐjø?Ã_Å
iC?Ð9ÌuË€?Êj'<z|?•ŠX'š$b?Ÿ`%ã"(?ç6ÇHéî?ɛ¹S0T?Õ¤cï`?°ôUüܖ?µ¯K͔æ?¡qr"49t?â¿DT~î"?±ÉMP2 ?Üù'åo}^?¯Ää€ZžÖ?åÚ\N×Ì?q²}~e?àüºª'Â?¯€°÷P¦X?Æ4Æ%"¸Y?·`"Þä?žÅQhæ9?–õŠ ÎÙL?é|¦t‰(?¹#'`­?É`Òòþ?Ý$là—Ê?—¿ÅÛÊt6?¦@°tQ‹Ž?èéÍJdìØ?ÃèɸEVK?ÉNC¶IcÝ?©˜;'ý!?¶'ÍTVû?¢{j?æÚ§ŸI?­·F3E[?Í/"k8?­íê:Ý%Ô?–"Üóó?*D"ê#?è¶5†Ÿ—?­Ù•¢³šOTHER4FGL J1316.1-3338?ãY}M–®@<ôFs×ÜÀ8gõò`MÀ;ˆÏ×CHT@Ÿ­"Þ@GØåó?¡õ'	^Ú?²˜Pï0Ï×@c3á®Ü!@…Våb¿ÐÒ¸©)¿ÝÖ¾=<÷W¿å3¥´Z@¿å¼ä!}(J¿åUK Â€¿åZ‡5DAGNfsrq3FGL J1316.0-3338PKS 1313-333?ïÇݗJ^ô?¯]V`Hó?1"¸¤m ?$€ž"h©«?z÷ø¿*ã?¯_Hd¸¡?ïå~)À]?h‡›Ý%?>f¬é¡Ô…?H¨¾;ò=?g¬CZ<Ë?dcó-iR?ïœ/kR‰e?ƒ'ºN…ø?\|Y=n*—?`5æ'ߥŽ?…d™ù	‹?'MևÓÍ?ïõõ:)F ?9˜X;Ø?"NVIÔ??
¿3"a?QÓAgÊ°»?8[\gð-?ïē)+â ?;½EpL™?<2Í
²Œœ?T¢"·C?{ó>¶ª¸?Ž•ÄÔ¯?ï³ë»'«?€Îåòˆ×(?NïÔ¡}8?_Üy"Ðs? –tÌ?Ç»UôN?ï~Ž­F8?‰ ?ãM'?c)³2"ù?j•®±ƒÊ?‹˜ÊLûí]?‡Ö|2‡e?ïé0è?Uf¶Pˆ%w?5~ō '³?&2Y!}nP?d7ö$€±?TtZUnAGN4FGL J1316.5+3013?㩏PÈøà@TëQÕQ×À;¬ˆô'À<ÿé]&KÄ@e°ŸÅ'¬?ûÒÂÊëK=?âÀžìå?қ‹vÁ'}?ö;¥wô-d?þ•ùqE'†¿ïý.)7?ïÄҗç貿ìV́¨Œ&?Ӑ¨"C3¿çZüۈQs¿ïÿ^Ô÷"AGNbcuRX J1316.9+3014?ï@¸*d"º?¯.éU!M5?eæ/­b9?pwGƒýô?•,4ʸ?­ãjßLK?ïÍq£cû[?yüŠ¬ÉÏ?KLÒP R&?WV‡÷B³?uݔŒ,H?vä8zPñ?íà!Å;w¿?¢ÄSå,?u虴Ur?zCîËå?¯@ÐxՉ?¡˜Š«ä ±?^Ý(?pþÈ\w'š?t™ÆxguP?g"LKG ?	U%5À?gRDt9êÞ?îϒ¤TU?°¸áD&k<?tÀ¸‡:…Y?t ERï? n¾¦MÄõ?°€hôDÚ?ïdfþ"?–@}b€ñ?ebà&ö(Ü?k44Ç©>?ÆÄ0WFõ?"×ñtöà?íÞ€èô?¥´ßÖuà/?|ថƒVE?}>ã'SQk?µšõûtsþ?¥KÜ%¹
?ï0"pµŸµ?‰Ó´²¬±?yèІö?·¯).ê¨?"s]ßsw?"ÚIxt#÷AGN4FGL J1317.1+6613?ë'ëòyQ@IYÝDUGÀ;D·éæ¹À<ÑÜKÅÑ0@ƒÁRñ©@|l—ØÏ:?ÂFµœ¬2¿§¨¥ûý'ç?âN¢?Zˆã@ÚýA‰¸%?î†@áDž»¿âk
ÀMb‰¿ê

Dý`¿êjˆ¿¬¨À¿ÝAÞò"2?r<TçZdAGNbcuTXS 1316+665?ïÊ]åʅÜ?¢½_Yr[>?Oè¿ÆŠh?qXŠøÿt?vðäªà!?¡NŸP`í5?rgs?ƒä6hbÂ?^ãÚ;'€µ?eÛÒ-ô­?"Þ›<.?€ÞþsPE?ï%21L9?ˆ³6ö!´û?r""Ú90F?pn— KÓ?–Ñ	|	½?†r>dø?ïÖ録;¸?Tî_æ7á}?Vî¯)§v?DwË¢žs?mŸ¤[?PïöS¡N?ïÎ#‹Â¸Ä?uý1ÿ%?TÈ:,¨ÕÏ?LϨYèê?s¼+‡Ê¼‹?tËö¸–ï?ï´RNù°?œ}ì=K'*?j³/2ïÁ?yåYcY"Ô?œ"Ø3_?™uûzwNó?îxiÿ#â?'cÏOŒnß?€O
´å"?yPE0lt"?¤e«V_§?'<(ö[?ïc5N7èÇ?xZEi£?u]â±×þ*?hÄ­ÀTZÖ?Œƒ»!Xß"?s­‰'AGN4FGL J1317.6+3428?å`ó¹~Å@T0Åë1;âÀ9ʵ™ª`'À<jz4y"P@yáäáìo@÷
=p£×?´Qbޜƒ?´Ñ^¬ÞšÖ?üëNbc¢g@Vð|ªK¿Æ!Ï4`¿å};?HÜ¿æÔXÖZë¿å¡ŽàØóL¿í+™
þ`Ä¿ïâfê%xAGNfsrq3FGL J1317.8+3429S4 1315+34?ïÕW†ŠÚJ?¢¤ÂAÉy?Qm²aØ]?|¤ßbn'°?pøõ
ŠÈÈ?ž,âûÒÁ?ïÔapˆS?u[&¤Rò?I¯æjý?UÂÑñVÉU?rӋšâË»?qvÎ"Ã:†?ïm§`+¹Â?'–HtÄù?W'¤Q•?BÍ°ä&ÕÆ?Ø™¹ÃéK?'õô¼À?ïï>gÕã]?CP*OM]?Q·xãÓ0?:"éM-÷?O—p‰K½?5Õj·ù3?ïÖ¹UA?uF׳»Bß?QϯÂåÿ?Q*ÿó–ÁG?p/iq€_?rŒ¶(½Û»?OG՛?‹ÙڏH«í?S}ß|ÆZÞ?a² ™À•c?‹dð5*ÛÖ?Šîù('Ÿ?ï:
<fZ?'}È߀¤B?`«¡Ã,©?RËé¡Äì?–©D=ŽÚ8?'f¯·h6 ?ïÎaˆõÌ?cÕkF¿ëß?kÂ(ø}oä?]łgŽ-¥?fuR'Ä?S(Ó(öŠ1AGN4FGL J1317.6+7450?Ԍ°ú«¤«@E<³åuÀ;'mÄÿxòÀ=ŽVox^@W"f1bN@_^4h½?ÏÇíÕ[È?Æ(t"OÓ}?íëù¸¾"?÷õ±Ím¿±â˼¬n3?à:õ¿ÏÖ"î9.¿ä©L•£¿çë@àðÆ&¿Ó~/?‰AGNbcu6C B131714.7+750402?ï>Ê+ÃäW?­ïƒm2]?ky}e ?'ç,ç@Ù?"·ŠÒH»?©ØPv€ˆþ?ïsÕº(§¶?‡¬(CiVô?p0ÓNÊ}?r/<ÝAÁA?Šò'Ә=Û?'R…IÜ?îÝ
"ºÑ?"!ä¹úù?Š
ŸZ5Ç?Œ¸z{nj?—Wï¥ö¼c?†ãýÉw‹Z?îùõC°Ñ;?wÞ*œ&?'¬‡ÝÚf?rwû¶Æ0?{VÎl\?jê¹sˆö¥?ï	ûÆ#T?'‡ßC-7'?tb0Á¶?pM—Ì&i?™æ?¿§ƒ?¿¢·¿K?îfG®Pœ? ½¡d'î?ƒ/jåõ½Z?…_gց?¤Ïª_«}?š«@¦‡jw?î[	;%?™IB½_‰?•&*Á\?'!G/†1?¤T<X¥ýc?JSŸà¿?íÒè(•?&ü0L)ø?^‹ðqi:?‡†iE{Ъ?¤"9õEò?…_ÏWóZKAGN4FGL J1318.1-1740¿ä=dSÞñµ@F]6Þ¹^[À:º¸ÌdÈÀ<fèQ'N@ìË]ë@þÑa‡•?È~ÓD¶?·—
ž¦Ñ?í;Ì^èã@¡ Lü‡û¿ê=G‰+M?ïëÒá长êÀ|1¿Þ¼ŒxHæú¿å)+<Ĭm¿ïÿóÖ&ãAGNbcuAT20G J131808-173536?ïz†'vç?ƒqx™hú?X£¼&(?O­òaN³Ñ?ŽK&ÿO)T?'†ÃÀÁ÷?ïÏ©³Ã‹?tQ™ú4]ƒ?N¹"6‰Ç?W~q_È\?tT¶ð¶Ç?p&>fðµl?ïaOõ"?~®"Ì'Ž?jü@½"T?h¬Ø3ßà¹?"Î8&?{-xª$òú?ïX¯=½M?k¤†"Ÿ²ø?x•}È[7¯?WÓdçñKs?‰q§cæí?fŽÕDmÐ?ï
ĎºÃ?¤ÐÕ&)ä?iÓMʂ'Š?cÞS(º=?šÃݲD­¦?-õè'?ï[~]usl?'qÍZÖr?aA}Þu?h£ˆ¡[#?'h=Š´?Cì»k?î¹9Œ	l?Ÿ´•èAð?{XT÷?{ig@aµ?¡e8q" ?‹Zv>ÞÑ?îk*Ë°˜?…a¥}'ž?‹º¹¾–íÝ?r¼cÏ,€k?¢^¤×äx¨?¿O1PºðAGN4FGL J1318.2+6754?î½úü#ì2@H±Ù+áÀ:âñ#ôÒÀ<ö1ø .@ʁðÛtÛ@"d¼B;?Ä+þNå?Ê'€EŠ¤@aãðÕÁ@Ÿ
qÈð¿Þ˜L<™Ž\¿ÑëŠ<¯]Ñ¿äiü¾, ¿Ùº?–më¿ìE ž²´¿ðAGNbcu87GB 131701.6+681031?ìÓ=š6Å?Ζü;$nI?§ýw-êç?½½5Ä̽?ªË«¿Ð?Á®.—ÿ î?ïßy~µ×W?n€-LíV?A;aÍ?M<÷ÔaŒ?l7¾™Ž:?i21«Ë¬±?ï,"À?'	qÅt{Ã?Ó4o@?"ʺ·'?"3n¡¬?‹%«zÌã?ïòUŽì†??<Ñqs
,?DÙ«Tü<I?*Z@Éi·Ò?Pè w±I?7'ß÷5Û©?íD´O}k¼?à àö$‰ø?©€™-é]?·Y4šü	?¢4!؈eì?±5'	â"Ñ?ï"ç"bx?ŒÉB®Å2¡?TÒAg¾ª?`4gړ?ˆkñYÔ®?Š‰<¨r'~?îy*ßã¼?˜b`ìU³y?Š´·RKn?ˆ†bêŒÏ|?¡À$-<ìH?"ôŏ@Ð*?ïڋõJ<?[ünY¼J?[†}ù!3í?I&z|Zk?g±¾3@ñû?U`ÌÓµ¤AGN4FGL J1318.7-1234?䆈jûª@HÞÆÞvB|À9ÏhµËÿGÀ<BÛ·K[H@Õ'*g@'Ú˜gjr?µ¡N›Ä?²²Z@úW[?ühMÇ3/Ø@©vƒ¿èŽ?ïûv=žñó¿ß%ôñ¯e¿ãÚüȼ¿á{lB†Ï¿áÈJÕ¿ìQ›žV—¼AGNbcu3FGL J1318.7-1232PMN J1318-1235?ï»NwÝ1I?«ÝM¾óÈ?UÉê•Å¯Ž?y­b…ù?|æIJIÃÏ?¨ g/W?ïѦ)—K?v
¬—td¥?NÖ"Ú¡H?X‡iäõ¶o?s¢jf»ÌÐ?ql'võ¥=?ï«uR:#?u·ò/íž?WÒöÞtd3?E
%ç
™?'(YÄL4´?tÎ%ç?¾?ï\¡Äfï?gøÛ¶ZÐ?|<˜7rö«?Vhz3g«?Š¹qó"¾ã?cÕ*V"F?ï³n!Ï;E?¿îãA?`ý"˜©?beËÉ[?~>𨌍*?{`¬ÁÖ*ð?ï^†<çßD?ä@†Ø̵?dâ∬ԍ?mžS¸ð?''Üæß?Ž)ȏ÷‰?ïvûy@?€±õEèÉ?e
­öôl½?d»ÌÂ	~?8՜o°ê?}ös‰‰J?îR'Êûð?"pŸíÌ?'@y.úpG?t#P›²¦@?¡½Ê:÷!à?€S³¬ wAGN4FGL J1319.5-0045¿í҈äs:=@N¦ùü°À'À:nd-§8À<lf/	@ؼKV@G@ÿ¤?»L·Ñ=ö¿‰ò'­gë?ÍåÑ*ªx@i?%3?ïü¹>z¿äAèÜy¿æŒížÔký¿áXl"h	Õ¿ïü#!BDô¿ë‡ù(ujAGNbcuPKS B1317-005?ï¶s«Q?¢‰Ö6²V?~d'•òÐU?¢åÀäŒ1?Zjz·G$»?P¥Ãg*?ïÒõúSÔÐ?wžR&Ár?Jxx5"2¬?^?'ª‹PÎ?s5óäâú?r÷Kh@«¡?ï¢núVV?}k
Í|â·?m¶Ûۀ?wsµò{?ísô4?o'"ôê¾?ïÀoÊpڑ?\.Š§\£?eë3©s?K[çãâKI?uG¥1-™ž?V¤B#¤?ï½ï,{¼—?œäÒȧ]®?szñ-?V?œìý$ö‡ñ?lÝŒÒ?dvœä"¨â?ïoQJ[ª?"'H#¾¨?Y.	¼åù—?e=0F ¡–?'ö!×V™?'eW/­:ã?ïd'9£º°?'³¹¨õ+?rHÖ·H?vµÃz˺?·F3Þ,Z?|õv/Kbû?ïF£ƒZñq?{øðž?€rˆÐ?kÇzÌ#­x?Ž9¶Œ.ý?t!G!'%AGN4FGL J1319.5+1404¿Ù=?Ë
ïŒ@RؒyèÀ:Ó!ž¶9À<™>ÔI™@øËagÏ?û߶må·?Ïâ+™5ñ?ÐA´ †å@¹	k¹Œ~@v®óH?é¬
¥0ç¿èæä:§›»¿­÷Àkj‡2¿á(ŠÎ$»¡¿Õ/æ5T¿ðAGNbll3FGL J1319.3+1402RX J1319.4+1405?ï°ý¢}C?y†·/OЂ?Z‰({}ހ?Tv¼'Êtç?€o""ÙMw?vp±Üšú?ïµéYîÖ?xÞ¼"1?Tõ3…ç…?V//à›ËH?Î1äš?u¡.8Ÿ¹?ï6«]dÆ?†|à¾UÂ~?k@ƒõ¸¿R?kšÜ=­é?•ÂŒéX?…vu·µ?î擏`Òö?xž'v¬?t;,P"ßÒ?Yí&pÄnž?žÃðC?wË'´6—Y?ïH%L"'?•ºÎIX÷Y?lïK›£?bYË~ë,?™Ùú_t]?"Ðkù?4¯h?™lIAvô§?iü.lØy?t&,1Ï?™¤¬ªêæ?—^™Àb?î&E3»Ä<?™Â¢R?|_ÐÝï.?|«_0¾l?ª²ª«z?˜7ÂpÆå?í«¾ñS%?•)ՔÜv?ƒ,£e?s0$ÇíR?µ^Üv#wó?"åÙpñ›AGN4FGL J1319.8+7759¿´Áç(÷"¿@C"{¢7ÍÍÀ:)6&,ºÀ<ªÖR5W@¾Ë$V ž@Y©qÛ?²"`_;Ná?Spaù.@
‹éû†Éˆ¿åÐ!ÙC©¿Îd"i®ðC¿ä΋魮$¿àU<þ
6Ÿ¿ßÐ`zn±¿Ö Uu}ZŸAGNbll3FGL J1319.6+7759NVSS J131921+775823?ïá¾õQY?«¶p?I[?="7á©?s=z?§Vç?kZþtSÕ»?©NîF6s™?ïåê÷tÊ?k¹'?:¾¹ZP8?GZR²•%Â?f¾!ÀÒh?f«뵪£?ᅣþéà?n\+j?N'~…ðŸr?6Wfg#r?|x©À·?n*F&?ïì."¤?AÑúø'y?C€·KU?$L€Ã›Á?^5ŸÐ9›²?@Rà_-ªÔ?ïöª'ä»?E "iPH?2j"'¶Óï?!óF|^4T?L ²81?Bûòrëïá?嬨ê?ƒցXs?JÙXäß?W0¤Ê¼‡ž?ƒ±ïôªê?€4…{$?zÙ?{³•-£ 1?TñŽ­Vt?TÌ[	|Z¸?‰<o›9?z‰wÄz?ïÊÑ´,?`Ç£­Å¦¸?Zñ#
Ì?AÃ`"K¨#?tz}ƾŽ›?^aYé‰"AGN4FGL J1320.7+3314¿ï™Ìð3.V@TM*®)s—À:ÖÛÃ	ÕlÀ<€ëLê"@êØ¿IV‹@g†
¢?Íía—ÊŒ?Ò±×~¶ß?ÿi±Y©¿'@(¡ ¤$ã?ì†X>…vÍ¿åÎj[¾l¸¿å­u"›Y¿ëÞ`]Ï·¿àù«ƒ¿ïÿÒþÀùAGNfsrq87GB 131814.4+332742?ïÚäØ\M?zː+m¬U?T‹	÷Ž6 ?b%/ÈE?jÕ¢—m½?ra[pZt?ï° @9û?†L½ZÚe=?]ôÖ
¸¯?nfrŠ•?€Tñgïz?ONeti+?îòÀޛÆ?'ö2oë¨?yöz1RÀ
?€[þp)ÿ?›*Ež¦»ï?¤Gu.?ï–Ãa¥G´?h.˜P硬?jyƒ!N®‹?R4Ë=úl?ƒ°ÆÙ1X?eðy5À;?ﶯ{I;?ƒ½F™'Í™?`'ޓå?bÝJ¡Îl@?|›=Ù¸l:?Ȥ2r˜¢?ït/c<?¥¢œÖÒð?lD¬R9ûÓ?}nõÓï']?š(䁝š?£§ÉË)?îhe½|«U?˜"¡Eý"©?Eó i?Ô%"Ýÿ?¥8_S2é?–¤—Ž!wf?îql‹»×Ô?Ž¦árúˆ?†¡(¡b?uÙ㜁/\?£hòXˆ¾f?ÅúÜ»¾nAGN4FGL J1321.1+2216?çÈÞµ54@Tlºˆ&«À8ŽÅâÍÀÀ;°…ù©¤ª@ï°¨ÔÊó@@gc¼gû?¤)0N&v?³Ú6lΊg@Î^'lVj@rø_¢¨¿ÕÚj$"¿àđ"èYñ¿åG˜_ݶ)¿åž@ÈG,¿èÞê¦ÒgA¿ìJˆ_	¥ÆAGNfsrq3FGL J1321.0+2215TXS 1318+225?ïá‹7x‰¡?u
"ÿ¸DÈ?FÑõ«ë7:?@DB"»4?hÀK9\?t‡+'­?ïÉ\wFª×?vUÆ_²-?LÍÁžòŽ?Uº¯ä•³‰?w¸¾1¬?t	þ-ÝPÛ?ï¹ÍTӋ?qüf|J?]©uiNþ?`DR80Ç?{¯æ꒫?köç÷wO«?ïïK!'u3?C¹9Á¶íL?C˜'Š»U?-‹ÄîSԗ?WÞp×b5Ø??b@-Ö?ï¹C6FÊ%?w
dò?Us[/¶Z?RßÞ!0ðÄ?~ŸOŸê?uir·$À?ïxJÊ{Â?'PÉ,j}?Xc'³nÉ?f£LØÄ$y?Žá'‰9ƒ?k'ã1?ï‡a'·?'^
ŠèÚ?kÎêۇÑ?p¨T®"8Ã?‡HämBL?Îÿ¿ÍX?ïØÇ)Ó@¸?`ï:Ac²`?WUe@+S=?JڄPs>H?kŽ#hí®´?Zm±¯ËAGN4FGL J1321.3-2641¿ï±.€Æå@AØàÉÙÓFÀ:ب)À<L[œÞÈx@bó•8Œ@;þ¦c¬x?ÀªãƒrÁ¿¶B³-êI
?öª¼¤¡5@Tä©~>¿Ï""ÜÉ9¿é1àþ¿ì'ð}V¿ŸPg˜âÜÑ¿ç ÕÍýNu¿ï÷ŞÛ!úAGNfsrqPKS 1318-263?ï—EÔ_?œqT7L¹?ql¾~?›¸ä½£Fé?¤¼O‹Ša?~ÕP•^?st~½Rå?…R\Y¢Q²?aL,|Þ?ut¯KÕ?€‹UPÄ߈?yW–äŽW˜?ïãR™€?Šd$‰û€?r4‹?t܋¿bí:?˜žÑ{ƒ1?‡×îÚaâ}?ïu"
?vv–åS95?j"RF¾N?U†IÒëK?Œ.éw}e?sþlšn"ú?ïC6Šosð?'…¬ ßˆ?zH&þ#3o?zåncÏ­?'$ø¸?Ž?\ÃA·?ï+iGÂ6q?š\CÆÕò"?sâˆ'a?Š>«|ê
/?•šTT®?';Œ?î0¿
Awo?•N5®gÐ×?ƒ,‡–6‹¡?€²±¬ì ?¨(ízk¨?"ؐääý?ît†\ƒ?•™-ÿeÒø?*¡Æ4?†‰´P'€e?§Ãf·8Ð?'®Ûˆ	^AGN4FGL J1321.9+3219¿è–"tˆà[@Teˆ±Ù+À;IÀÜԁÍÀ<¸Hi%]ˆ@»Fc'ŸÐ@À
¼%/?Ål¡«¶Ó¿–[߂d§R?ÔÌÎzKö@ä*m'ÓÒ¿åV…þ\;ë¿äæœau÷¿çSˆ]‡º¿ÝVÀ	¿æ\C'‹¶?‹›Q:ìKAGNbllNVSS J132159+321903?ïØ-׺ͭ?qwk#Î?@t¿³G_L?5/&ï£?qÚ|+ØG–?pÌÛM¶œ«?ï˕F<"?v\x·Xê¥?D½Iúa¬?O§þÚӡ?wº—ç?t¿¦ªîe'?ïqPh‰g"?"	™‹©+?XÛݑa+?@ÐîÿL«?H5Éoå?ƒòðï2$°?ïÃ[¬Ï"?\€
ŸWv?R+Ó)ž?:o̎9Ï?yÇ4Éi¢§?[b&~óê?±|J?ˆ]†ßPß¡?LÑyÀT?G=!+ë'?…Ž¶'¡þm?‡w;¸ÍBg?ïkT"×½í?'†èÒµ?TááͶ?_âU\N†?'SoI×
?'1èóX"?îËêM!'?'\R ½¤?e_ÇÈÏdÉ?Y
~XR€ñ?¡ë^°ªüD?'Î8\½Æ?ï[ý·*?RÎøÙ•?nh‹Â\»?^Ú|W{QY?˜gnøP÷#?€Ýå"ÕŸAGN4FGL J1322.0+8317¿é<aÖÅÛ'@@ã×<'W†À:\Û¦"c§À<@–ÉÁ@!š…Ò½R@èJה§?Á<´ÿ?Á¾z¤‹åý?üà·õ¥3@Á?à뒶?ã;xçrj¿Û®qÊG·¿æžÍë°½£¿àÁJ³οëù®AÇJ­¿ïýR†Q¾AGNfsrq3FGL J1321.7+8312S5 1322+83?ïÜJ~Sm?d ,EXNÌ?R‡ÑÊ}\?G|ÿ2Z}k?j³½ËìÁÏ?aqݟü1Ü?ïßGã<¦?nŒ젘5?D½\:=;"?PÍÄ­½<µ?k‰¤çX?h'é™-Xi?ï¥Z$Žª¨?{4ŠðŒ'?dØÿþ*ýU?j‰!$[‹?s6Ù²ð¢?wº8Ô"Ñ?ïäNçÓa?Gëtkh´?P|wObØÙ?0Óȵ9¼ƒ?crÝ	áKN?DõU*UÓ?ï³VxK"ý?y8ý¸v'?d—¤‰Ó!?ZþÓÍúv¸?|÷ø*cÎ?vdI¼p¸í?ï¦ó»4Z6?ƒ™äçy?Qü÷
m?`ëT‡vÃ_?"öÇ Õ?—ïÞêB"?ïf]g9J$?"{㩜ÁÎ?lWŒüv·X?oÆmOHC?RÂîÈ7K?€®À5"k?ï¯àÙQÈþ?g•f¿‰¼?gze~¹^P?Px>(ÒU§?|R`Œ%Þ?d:AGN4FGL J1322.2+0842?åðނŠfÿ@QŒ2 f<uÀ:gég7F¾À<~ˆA'O@k‡}'@_`'÷–¥?¾&4ÈÂÇ¿—©Ä—ÌÝ?Ú5˜}ºÀÜ@"{½™Á¿Ú¯Þ|·â¿ç–œŸ2ŠÂ¿â.5!õÉ¿Û:…M\T¿ìrH½3«¿Õ±$ûŒÿAGNfsrq3FGL J1322.3+0839NVSS J132210+084231?ïà‰'+?bºOŠ{J?MĖCÛ8¤?@
o'/Á?hJ‹ú'¯?`ak<Õl…?ïÞV6Öo?si<‹èg?>ê2·Šy?LÍý˜ÌÃ?mÌwåÜ<¨?q"y\æ?ï–3aðû?€"müŒÛ?l÷²òb¶?s¸.èÈAR?ƒtuKõ4•?{ÀGjç?ïç|ñ˜3=?G¦H­k3Â?KLŸ:˜#?2Úö=‹¼ï?a¯îe
ùÐ?C¤"1Ã?ﺡӓª0?tÞ½}3
r?ciÓGÙ(?Tfk©ý+?xú,¥|0:?qúSQŽx‹?ýsß?‡°Ýæ¢!X?P!J¬çI9?[äÔ@ŒŸ¥?†Ž×Vð?†7ùƒžŒq?ï9B\Øs?ŽË^ïÑ>?táòW¾]?|Ø¿ùd6?"Ÿmè¬
?‰uÕԏ76?ï»+O9#7?fgö}°
?c'8ÁLo?R
þ6ügV?xà×‹Þ?bµ˜ü"V,AGN4FGL J1322.3-0606¿ë_×"ˆ@K÷²VÿÁÀ:óY'BCÀ<´¡õˆ­¹@@ ?û4ï*Ŧh?ɂ§Í"]?Ö¨B¿BJ¨@3å	Út?ÿl¿y'3¿ïÿúVrÓ\?ïÿêњ'ç¿Ô	B%¿ÝjwØ~±·¿âYDàá6¿ïý'Æf>AGNbcuAT20G J132219-060619?î"涥:"? Jgª¤§ì?"ÙÓˍ•Q?Œ)4f?ù5?›‰U^L1?š›ye!'?ۯ
<?£ŽVH?'žqà©4?–ËU"·%©?›m¡^×d?"IÍVôÿ'?ëŠMÙ6C?ª†™ÞI24?«¼Lö–"?bÛ²çË
?µÏj¼ÛiÓ?¥[ÅzRiu?ìOÁº±''?'~ùPˆ?¨·F¤e`¾?ˆñæñ¾?±&N֌E?‡¾§5¶?î6A'£_?¡;¶¡}˜Ñ?›cÓs‹ç?"¼O&-ç?Ì[÷{?—çGŠH¼ß?ëç,BWÝ?ºí¿SÆc?ªÀ§Ï'Ž?±ß²˜†-³?³fJ¾­N?«M®±õ)9?éã¥ä" ^?­Nm…ÆQ?µWBƒ C?¤µ¿RÜ]ô?»‹Âš³ŽÒ?§mÖ
¼vÖ?èf ·'u?¥>ˆÎ[T?µN–à"ì?œd7¦Ï&?ÃÀJ
üS3? Åy¡u"ÒAGN4FGL J1322.6-0936?¸gûíÅÂw@J?^g"dÀ9.ø6#
À<"*M±c»@SoЍ@'êÓ²š?­Š¿q6	?¹¸A¿+é,@û#š8ûÊ@«AOÝ8¿´"ôxA¿ã¦¡Ÿ¢r0¿é,.âkšƒ¿éŸÎ!5¯º¿ç4R¿æ@Î&i UAGNfsrq3FGL J1322.8-0938PKS B1319-093?ïús&úPû?3{«+? BÅR@–A?D•Rä8Œ?B"³A*Kâ?1ƒb‰ƒÀ?ïÝîÞ£¤?nP»·Ú*?AFsd'—?I&@×A¸
?mɏÎ85'?j'wôÉb*?ï¨-ÆQf?{óŽùÉ­M?d=.JrjX?o͓æa&k?€åBèŽ
?vÅÑ 'ž]?ïûM/L'?'ÐÅ/Ù­?&¯¶c¡\?BZªÐÌ?:>«Zõ_?#"j¾2/¦?ïöÖ-.]?G"%¸n?&\ƒœ«¿…?8Ïñùk"?O*xʓ'?ESÊ2rcq?å8¥?'æËoS&?T%ÜIHɟ?b'žûd¯?‰ÚK8Ù'‰?'X@(¯?ïh(<¬{?ƒãåpô;&?rMX²Ðu™?w¦
£ïtG?ŒÏDt™Ç÷?퇕¨¤?ïòX™
?J"YÌ?B$Skq£È?3î/›`Õ¹?Rå$•â.!?Ehƒ;¸¿>AGN4FGL J1322.6-1418?ïÝTovŽ@Gð*#¿ø©À;wëÒK'ÏÀ<°$?ziS@ d°êöY?ÿ)¸`.>?ÑÔȄ=¼Ï?Å´!ZBÁœ?õGuàVíM?ôí¡
Ò
¿ït†ŸÁÑÇ?ïüÖ 
L	¿âL€ Ì©;¿Ý3<mn˜¿äô'Þ½¿âÍÐØËÑAGNbcuTXS 1319-140?ïz̧øý?š‡hJ´\¨?fÃ|g<ε?pÖöe‰ì?‹›öùÑ??—ŠÒý–r?ïC?—½¸—<›\?€݄oÛÄ?…h]
V'¤?"\uhâÃ?-Øyýú?ï,Yí?£?ˆa÷\fŠ?r™™¯ï{?t$ªu/?•Îu×8.Ç?…ù1O;r?í0ä•&©?á8"…³?žÏ_ºâ?€Ù‹bžF?­—1Õ"!a?‰ú¸9å ?ïY×y,?‰5ò'«¯?eóo$XU~?j>ô|c³?‡,ã˲i¡?"ò¥m±`?ír¸¨ÂEN?±tœ¬Øík?–'…ýpÞ®?žkrŠy$¶?­À²w¶ðÂ?©F–̼"÷?î›Îã°ò"?">et¶g?€Ä¢˜±?}0²{
x?¢> žœgô?K~¦^?é|E-å0?¦.Ʀ'Ý?¬T\Ó?šñ•ÿ½,I?Ã
%ôA—
?¤@n¾¦MÅAGN4FGL J1322.6-1617?íL%$9É@FöFñVÀ:½i&4G/À<€SM"î@FÒ̖5?ÿ~"ÐÜý?ËÈÕFmø?»@ö•H&4?ñ%HĔïç@QÉc?ïñÑ~N³¿é§ùä]K¿à/÷¤ç«¿Ödf[ÿ…1¿ãðý=ØӖ¿ïÿøãúAGNbcu3FGL J1322.6-1619PMN J1322-1617?ïÄQ"7?jã&jIã?IÊê@ At?8Î'"&?zžë]?ipLƧY?ï´ÐJkð$?wæ.=Jy?TÜ^:Ÿðj?XÖÌ5¸?€0a­&6É?t[š@ħv?ïoñÍbHõ?s''D¥?b¦×ýýÑ7?P¢5Ó®3Ì?YÖ¡ga?qWÇZ{°R?ï VjM"?tRVš±"¬?{'ªfÄMÙ?VôÖz¤L­?˜—J'}ú	?rÛb¡Û?ïÕãÕZ™?lå^O?VHx¦š2?H¯üŠ]ga?ŒÁxô[‡?~öÙ2…?ï&`â÷d.?¢
–éÒ?fÔÝv—þ»?j†íÉâV¶?˜YGú'"h?Ž¯oיÓ}?îЭQ²OH?ŒT=¬ÏO‹?l_w"§â5?d4¾?ï˜Ï?¡/3k´¦]?‹9œðp7?ípÔѨÿ"?…QG¢)V?µ†)­?t ¬-}	>?°Â¨ ax°?Œ.näuqAGN4FGL J1322.9+0437¿æQ7†ÈO@P'ò{xÀ:ïùwO¶À<™€TN5î@ L—ú³?ùnˆwÆ?ÔCÔýKp?ה&}˜1:@2äÄ:W@ʨ<ʋª?îÜEæ"0¿ìõ΃†1Þ?Ïb`\â@¿ÂôƒJ!â(¿æ5'ST:ë¿ïñH­ûŸAGNbll3FGL J1322.9+0435RBS 1257?ï™3˽?±Sïe£Õ?b珲?w"Le"E?š/é˜-µz?°­žRI?,h5@?…ª©dÒbo?`]‡~ÒÄ?c'å'í¶?"ySvÝP?'ÙÂÜb†Ó?ï=F(ñÄ?ˆÍ=1¥?hã:lsU?iñºDmn?•:ß
¼ã?†âÑFDƒ?î@<[j?ƒ°Ÿ¤†kÄ?;¯J‡@?eá<3úÐ?§­R4ào\?'œÍØôÎù?ï
ÆÎÊ ?›—&%BTš?\rœª›ª?W4~[«o€?œüUÂ?šç	ÀÇP¤?îø>Qì©.?›wÈ
0¶?pËýIåLÜ?yÅèß×[f?œÅ6ti?˜zO }ï?î~!»^?–ztx?q$/~'šÚ?t)Û%j½?¤ã—ø+`±?"ô»˜
çÿ?ëèVF'?ž»~x^"?‹g¡
7w¢?}<('Lû¨?½P[³ÁT?žR›Úñ»ŠAGN4FGL J1323.0+2941?'à~aX*@T¦}¿H€À8è[;ùÀ<ʍWkø@9Dü3l¿@êKáQ?¤p½¾x1{?«²DœxWf@œÄÇDÎ@º`@²w·?Ç2"åX¿ßð(‡ƞ¿ã½†]ҙ¿áŒé½ž[ ¿å>¨²;Q¿åwR|¤–MAGNbcu3FGL J1323.0+29424C +29.48?îô©—Šíý?•ït²þq??o–Ç8­€_?e¥ë»"'.?wô(<|a?"pÆ煊Ä?ìåL lœ‹?ÀZܯîś?©ø?$)ÁJ?¹J/yšj?§²ö× *ü?§ÁªåÂ?ëÉLÜbÓ?«õzŸo?"°o?MÕ?"fÐg¸«@?¼ËÌ>(üñ?ª&§ÂMÙ,?ëÊDo¿õ? (ȏÚy?¸ÌT˜7ä?³°óÍ?£R dG©í?€"
Mm^?ìãkÌP?±/4WíÊ?ˆ…Áþñ?"Á±G€S?µâw@Æz?¯µšî7¾y?é>à5½ÚŸ?Êa™'ÈqÉ?¹ùVüi?ÄýIAg~?¼§Â'ž?½]‡^rjð?ê@/œ6?°ó…uå¤?˜¸ÈÏŒ?'ØÅ^ï)?Ãæê1ƒýó?°QF¾‡8?ç«íÑv¢?³bÂ=Á?ÉÂHõ"É?²_Î.O2h?³ÆƒÑs_?–×ûg•AGN4FGL J1323.9+1405¿¼wó&þœ@Rº×à&EåÀ9æO"}ŠÀ<3PëªÞe@ cøÍܗ?û9AŸÝ€y?¾ÏiŠ2H}?Á­wÝ\<@í†"ÄP'@¦©øa{?螺¯ÀLŒ¿ä—P~"Ñ¿Þˆ…3[!¿Ïñ[øNZ׿ޠÁÁ€éJ¿æ/RY,AAGNbll3FGL J1323.9+1405RX J1323.9+1406?ïD^d©?Á·Ä@Ðï?–Ì¥LºŸ¢?ÁÂs?FÝ·n'c?2fÉrƒ4è?ïÒ` 7i4?uÓ˞Ã\Þ?JMH"?e•?S;ÿèW?s†FÔlz?s3""*¦?ï½+kàñ?k'B="	?Xa-ÿ,ˆ?der†tð?{Qþqà
?a7¤¸*Ü&?ïÇ<ƒØ¬?q¨À»âèÅ?t Á—=·"?SÍ8ÿ7D›?–þèäș?pÍ"N³¾?ïë:,?"¢·C†d?Z"´Ø°Iû?"žpMWè?N«®'g
©?;6øžßº@?ïw՘½?ŽIÔã±?\Ã7ª=º ?cèV÷¡l?Žr2ã²5€?ŒÒa8˜?ï I °O?wOúÔpÿÍ?`¼	
ÎRg?coøv0?‡Èëo8í¾?s›hð:*j?í·Ò	«-?åÕ^ /?‡žËYE›µ?p¨QÊ3©?®›,‹Œ+@?ŒL‹ì)UÜAGN4FGL J1324.0-4330e?Ñ¥\QJ܃@2ú&€IRÀ7®Í™{f©À:ØÆ;¹²@D*Se­¯@Äw¡!MX?£®¡†­?´-2<@à
quŽ@ô‰PKFû¿Ú=1cÐ4
¿ä+ïý©c'¿ç9m	Ö¶¿çÓÞ¿=˜¿è˜—;ˆ¿ç04{1ÐAGNRDG3FGL J1324.0-4330eCen A Lobes?ä&¼ÒÙ¬.?É/¼R£ˆR?¥¾ŠQÐ?£™æIå@%?Õnˆ¯ø'?ÇÓDbQü?éü1ùĞø?ÅÏLæ¯ï>?¿r_»Hã@?Áÿë+ÌPj?°¬w}?«Ë(&͏¹?ᰒÖ4‹?¶Š=ð1ž?µØó É?¢"(%/†Î?×7™Ý"η?´ê=òþ•?æïfµõ"Š?¬ŸR™"‹õ?´ù¦ÄY"?–é"{jÔ?ÉőÅèP?«OªšðG*?àGq"Ô?È
seÓC‰?­2ɤð»?¦(K[o¨µ?܆<´U!?ÇO¬Æ-?ãàs2§6?Ñ	T¶æ‡?КÃö9'®?ÏFPçy }?¾'S­"»š?»|˜±gA?ßÛ³âg‹!?¶&¦ g]ð?ºG¡^›?¥ãâó<¾›?ْ†yp8?µ #‡<Ìn?á	þ™?¶ÐnДÃÌ?ìBh°B¨?®ƒˆ*râ?ÔªÎl¬s?¸;¥0qOAGN4FGL J1324.9+4748?ç)ê™çG@Q³AáKàÀ:A(Ñ°aÀ<lÖ#£Â@+»öÀ'@#ˆ?¾äaéÔð]?¬PÑÿ'›?é"x¸xò@aŸ~àÛ¢¿Þ}³¿µ¿èüØÎbÏ¿çtøÀEªÚ¿ç8uý³¦¿î'âJãS!¿ïýNª‡þgAGNfsrqTXS 1322+479?ïòBkúð?s¿NQµ?At	+{z?h°ðX8—?RÁ#%:ùX?[­ê6Oª[?ïßó0Ané?o¢Ô#©¹?@¦'×?KmÀó˜T»?l/œ¦m€?k@óUn¼·?ï¹w´'ˇ?r7W`}.?YÛ*Q&#?_žÙ ü{?|Í[pôžË?o¤u)«%?ïô@[å®ñ?:É%âU?@•|³$VÉ?'ô¥W°?Ni9á9[?4\" ãã?ïêžðN9Ò?X²©DŽM¬?FN• šÛ?89ïtËc«?_šÔHÁ`Å?UGêB%¾?ï›é;?‰E1n=?TU\@YI»?d0†äjã ?†®zæc?‡Æ%l4×?ïwJ-¶?€ÕA­úŞ?a€QuÈÁì?Z!ÃGæ'?Í`Z-©ú?€§¡‰4?ï۟©…ö?^{ÀOÒÚ?Z¤ârb?K"c?g
þjށ?WlUʪ@AGN4FGL J1325.5-4300¿´ï­S^¤@3k8''À7~'æ!1©À;H4[Q_n@@`MȊÉ@:´œT^ý?'œÅ+	¿¨*Àüg£@‡0ž-}@!¯Påö"¿Ñ{%û'2¿çqÊÛ[¿è½*BsÂð¿å½Ž€á¼É¿ã1?=,±9¿ã`Æu(AGNRDG3FGL J1325.4-4301Cen A?ïwðÆ?‰9… ª‰E?jïkv[R?gßÜùZ"_?‹é,\‡ô?†«Ò³
?êü$ÀÌó?Æ°ý8zp?¹ÙØlãå?ÂìòÍùƒË?¬ŠUkþ?ªëæ´´»?ë^†Ï?¦õÙÊ+õ·?£Àۂì/É?š÷h¼2ôë?»+a¾È
‡?¤="üá°?ë荅‰?¢Æ²¢OT?¶ûEúƒ?Ÿ\
ÇùA?°v'a±?80'*²?íÇÖ½UOW?ªk¯	?êõ¶»ì?x'cÕ}-?¯*%µ ?©…?1¨ ?äÖð¨&غ?ÑÙ8Üэã?Íԏ8í‡W?Ïÿ;û¿åš?½Ÿ\Q9®w?½ð4½Ä=©?鱈›šzÀ?¯KÎc'÷?¨'ïÍÌ´Ì?žÆìoÅ?Ã/ážYá?ªÀ•Q£p9?äpðñ¢Í¨?¹YB[Å"´?ͬôjJ¢?·¾"ܦ?ÁE
~½?©Ùë:íAGN4FGL J1325.6-0227?ꊤX&v@M¤Ù¾L×IÀ;$­‹¾åƒÀ<¡Š¯@ q‡^Ù8?ýªHiü?йܚ )×?րB¸â4@Á	š³u
@,DeN¿ïþ"ƒÕâö?ïüA™þCg?èFp¢¿ÖµÏÅ¥'¿åˆqy‹¿ï²!…‹ÅœAGNbll1RXS J132542.1-022800?ïÈE®àӕ?y¡¸†u£¼?`8®•ñÄ?`ÖxkM`C?sÀÑt,ô¿?rÕ ó?ïpÃBúr?'Û›b?¼ä?s¼{\Fñº?€MÒzoŠ?‰ðñ–ǃ?‡›MS
ü¿?ï"éëÛI¬?n™ˆ>|?vŽì-ñn?xtŠ™1!?•ÿ€©'ô?‰±ÁÍxû?í¼õ5ª:?öDÏÄ¢'?š'¿‰á?…ÒƒqÄPm?¦öàé¸v?†I	█y?ï¡bñðPh?xwiª{Ü ?n<X¬,®á?dOG¹47?€-g§)?r¢ý²ÔX?à™»?¨)sÄWd>?‰Vž>¼K?ŸôB¯×? ŒP#??š'0®d%?î5‹Þë?•
®i_j?~f§dÂ?|¹ÞbÀL]?¤KCƒ	¿?'ž˜˜~?ë¬Ú`?¤Ÿéu3‹?¤ôÚãßåŽ?š°`rÍ?¹m&ϵ? /Vhn2ËAGN4FGL J1326.1+1232?æ¿í"O,°@RRwÄ\»ÃÀ;p`B_öáÀ<ÁîqbBë@ ŽG¯—í?ößùµc#¼?⧻Ðüv?×k…òž?ù!¨¬\ý@]cIP€÷?ïé`p¾.¿­Æñv–¿ê˜¶zzða?Àe­™UÑï¿Ó
Ÿk?¿¿ðAGNbllLEDA 1410672?îõþÇE?«¿¨@UO?kCÅûÂñ'?pvþèŒÓ?×®cfgú?ª5>|ò¬Ì?ï½ëºg‰@?gJx/wÎ?NQ'
ò"?X"Ϭ7m`?}?ð´÷+»?€HŠ#a?îNÊ­°c?šôOŒtû?xN|_®?{'%0*³?¨ëT–=?š6Ä´»¹?ïEö§;æ?xKvôÙÔ?cŠ	þagu?XòB´yԋ?"Ïé݊ÒZ?xƒCV—íl?îPCö`*H?¦‰F¼Ý(€?zø¸°W™?{¨u€èÏ?§¹á†Äà?¥?|ŽºÑ?ïS±ÎÒ4?"'ìùŠgo?btÄs'?p{¯O@¶{?";Eä+\Q?'»#»¤?íSf¿|­%?£eÄyù.?zÀR&yK?{Qò&%Á?³¸ÈÀXD?£
6¤uÎ`?îJ	é¸ÀÑ?•hA_?j=`![?r¦³S™ ?©½í‹ßÚ?"šü÷áKAGN4FGL J1326.7-0503?Ï?TeD@LXÅCk›À;ÞÈè;¾À<×ÁЈg@"æt™Z­?ù2Æ[™ƒÊ?××Õ^Á¬]?´ìU~6¼«?Ԟ$ƒBM?ÿŽÞëuj¿äÁ@ýv8¿â¿Ýѿ恽¥œà¿ËbFÇÇÄ¿³ØDЩ*¿ÔLw½PØáAGNfsrqTXS 1324-047?ïÌI2Š'?hH"†?7<Ʉ…/?&ÒS±"?xg¤öD0?gÉL¼‡ ?ïLRbÄÜ?œŸÀØ«Zë?p¨µ­L-?~šô_#V:?'K®T;Áw?—=âþVK€?ï"ã?ˆ‰¯?‰–N7OàY?[¸C"??LÜ$ïÔ?™èáD7?‰Tl´Ê?ïOª?â¢?‡8Ìn:í¨?NȦÜ6¬‰?AÏ{=ZA?'nÁÈ'?‡@ck‹ô}?ïÈ!ÂGŽ?¡
f2Qr?A¬,D(˜?4ÃN²_J(?Šó4̂¨{?]_ƒªŽC?î7'—ª?·ùiC'¬s?s‹ì ê/?†¹LÐ-Îq?ªq7m!?·C5ˆó»?îj3§>€?"Å"ÖXD?b½Iû:/?W@ö‡6?¨0ñâÓ?"ˆ	Üõ$_?ìaÚ<:ݐ?¦†õê1Ên?cي¿›ê·?eX…¡g?¼RaÈX/'?¦žõ-{ÿ¤AGN4FGL J1326.8-5256?ì´óʒŠÝ@#ÀL‹ÉÍÀ8"¶»éÀ;\hÑz±w@¡×sï»å@mŠaî1¡?©9è?U;­?Á ãd鹘@ÂÍáŸÂ©@ЯE¨UÊ?ãýߔO­½¿ß*ø…«¿â\¾™XV¿äsY(B¿é€ÞLQk¿ì5Þ>XˆAGNbll3FGL J1326.6-5256PMN J1326-5256?ïBz[e×J?†pG¾(1?jìq?`™ï<ÔÀ¹?"S"énV?…™fs?ï­½Dõþ?ŽjïЊ.?Lv"?°T»?VñAØÞÅ?'ÉL¶Ñ0´?Ž}Qà('?ï,[ö?|¿Sæ¨?gŠñê¢N?…¥üÔQ{?'É9£'è?‡†Að?ïµÈC{*?b••Å öc?QØ|}†íà?:'a|÷iZ?€>d?ËÂ?`õÁô
ÑÍ?î>ì&¯AL?ž
°ÉŠC?w£XA£?qguäïg†?©҈Hox?œíüé"­?ïZ9DDR•?˜ÿ¿«`?doÉHÙB?xòœ±þG ?'*åXu<6?–±Aá3ҏ?ïªOþ?™	Ãóì=¯?•Ã P­m?Žœ€ÎQ?™c uf?—?'M¿¯
¢¤?ïDçÅ:v?hI\Þi?eЄ…<í«?R0°2HÊ?"¨öÊE_»?}×ûÀZl–AGN4FGL J1326.9+2210¿ï½À"x¤@T"¯ÌáłÀ8à~֟´fÀ;ÌËQ¢Š@}YÏT;—@î,ëñ?§›¶Õ>¶I?¾L`RP/@]"Äm'º@¼]*}'¿Áç~~á–¿âYÏ^ø]õ¿æåÂ!M,¯¿æçÁz‰3¿éò¶ÁG³s¿æîè`Q#‰AGNfsrq3FGL J1326.8+2211B2 1324+22?ïäþµI›?^™¼UŽƒb?Q6$Ãóy?Gz{"1ñ?bÿf8Tkx?XåÄ*:‰?ïÂŞŸÐ?vPH®x"?S%¬î#I\?Z"roárÍ?yÓÅSú…š?rÙhrúXT?ï£^ç
)?zK(ØÉRÂ?e­¼F±?iQ¸—Q9?Èý?wÌËÆú'?ïÉ¥ˆe>É?Y½¤Oq?a·žÓšeT?H·ÖѺä?rQloB¼?SšëLÃhÒ?ï·Q"¶õ?w÷}…¶ì?aS[½²?Yì†?Ý2?{­²^™3ß?u+=*`ÜN?ï`$À©¨Û?'©5["á?a'¢"x?møsÄ?'Ö‡óï?™Üñ™F?ïLzo1ç?‹siÈàGî?r…@wc–­?t6ø´bï?'Ïaÿ-Úõ?‡×óÎA·?ïbmöӆ?||Ïvܾz?{)ˆ«²æ:?k WBðâ?‰Ç +ÓF?tšSÍåUAGN4FGL J1327.8+2522¿ãì%²ìüÃ@TjGG"#À;¢
6Ih)À<ÜS'ˆ@!S `Q®?÷_›ªcì?Ú±ÜÜdok?Äß	$ìÉl?æè$¬‡²ç@ßbݚÐP¿åJ›ÏÔ¿
¿ïÔ~ýŒ`?ì?©-‹S†¿ß7ÀÜ~œ?"?QyšJÄ¿ãX^èm½AGNbll3FGL J1327.9+2524NVSS J132758+252750?ïºß{óc?€Âs¥?M¨O*™"8?K¶ošÄö??=YUÊ?…ü"GÌ?g0Fªð?ˆ?dÎÅ?NZˆ­P?9?[€'3[¡?}qÕÆÑÏ?†ð³<ï$?î¨JCg€9?•MõØ"?[‰yX‰?Pwý‡ëŸ]?¤¢çF '?•>ŠO/Û=?ï‹ÃÖëû?pø¤†""Ž?-Ùìˆz?!³ªuV?Œš¾Î*œ–?pÑ2	>Ã?ïZò›Ý?"úÄ¢sí??\H"^5Ñ?Vâ
˜Ôü?'Ý4&Œ×u?"MBž£(@?ï25T'÷?¥'±ï¨y?\oÚEí³??qø§Ü©ië?—ò_ꇃÿ?¤W®ñþ14?íwÜ£¥§?  ÐúÁÃ?cÙ1÷G?e)Ãp«Ú?³¢Q`ž:
?Ÿæ'';w2?îÙ×jñ¡ª?ŽžWËAR?.,0Zr?0uùnÁB0?¢D‰5¸?Ž†ø*"@NAGN4FGL J1328.5-4727?¤4çr¨YŸ@-ã
£3vÀ9tµÙk@ÁÀ;ÀŒŸ5@ áWÕ©ë ?ÿù6Òúä7?µc`øh\
?…³'Eæ?Üój:±VÐ@Σü¿è8ÅÖՏ?îAdÿ‰¯¿â]"Ð_¿áPj¡3–Û¿Û®ˆ^]ÙO¿ØVÇaþͦAGNbll3FGL J1328.5-47282MASS J13284063-4727496?è{ÄDåã?ÔZòÔ7>?JÕÌDЋ<?De6 Ù«?ÍöÚ(É?Ô`ƒ™¹5R?ïÉéÆ,ʎ?|ÒÚ}Æq—?Q%»ÂãÆ?[ˆgì
?vÁ­ëÓP´?wàɱXš?ï¬Qúk
?'CFðì?l™ë(K†c?i©=?œ78^<â?'§'BÌÈ	?îx•,në=?rx ¬/?|ÖyÞc.@?^gÏ5Ÿ‹?¤ÛÝühÿo?}U4,/ó^?èä˜Õh@ ?ÒE•VÐœ?`7YÕ&Â?[m¤Z2Ô?Ì,¿CÕËW?ÒQ>Þ¯o¼?ïw1ê€3c?üŽ'qµ?^zÇÎã‹×?lOJãúv?Žd,dñ©?Ž=÷ºêª·?íË®=%áw?¢{'ç?{ÈwÛÇÒ?x;!Z
(?¯Ìân?¡&›ÀÓT?ìV"yä?–Ëus>?'"÷ªW=:?{¤ƒÀúä?¸æià¿)?–õk8|AGN4FGL J1328.6+1145?ËÕí4×@R¯_Ô{îÀ;q3JEžÀ<¶èÒ¼ÐÖ@"&6oÓ¢?÷÷'#'?ÔÖNád‰l?ÇðZpŽÞU?ôÏsÀÁü@©_àˆ¿Â¸G"£é)¿Õ¿¯'ä÷;?Àˆ]¥¢'¿Þ=—$Ê9Ê¿"uUËFò¿ØY9W9£AGNbll2E 1326.1+1200?û ®]?†Em*Lp ?VÇá5¦‰?L.ÁÒÜ,Ú?…[¨I-û?…œ·%m8?ïŸé	Ìæ?"é¸áuŠÍ?Z`­×Ώn?a@ëzsŸ?"¹§Öô?'§Ï¯ƒ¥a?ïªñ?rôVc?a€¾ü´á?cW~+¶?œ×'Ä*vR?Œc§9r?îú"òâúÐ?0=²|
?U_±*Ì?D"ãZt#¨?Ÿk‹¢»á?LýsXž?ï$!jç]$?'éþƶ¸?f
'yð~ÿ?Y¸åÝm?˜º€LŸ›?'XîƬ(;?ï
TvqBÛ? ÿÒº¿?h]"—ÇîÕ?{s*CÉL?›IÌå'ãÄ?ŸhÇrMƒ?îK¾:wÂ?–2¼2#Re?hªýçn[?iÝrï±2M?©¹o?+x¥?•¿шÙ?ìÞeã¬Ì?›L}Š†?aĺÕ_Š®?\QÏÆ?¸~«†ñÌ?›<Cÿ¾y"AGN4FGL J1329.0-5607?îh¬º'>Š@y bvÞÀ7ÛjUß/¦À;ßTŽÍŽ@ÆCß}Ôl@Ì=s(? ;~.ˆB?½±•¹»"*@STâ°cà@º•¼?`é¿Æëðÿ\+¿áŽ›¤5Ôοå‰AAé¯\¿å¤º|h¿ëË7×âr¿åÀ~SÂöAGNbll3FGL J1328.9-5607PMN J1329-5608?ï$«}i/?"Hœ1©?kmÞКÈ?f;*Ç"D?™-®Ð<·Ï?"\ÌÕHUá?ïEÃ/X÷Ø?¡%"캯?RèkÏ´ñ'?aYDh‡w\?–V±Øú? ÅØD'Ät?î.Õe¢œ"?Ÿñp$8?š¶³ò›a?–¶-áÖ{?ŸnŸWåk?•±8ˆ?ïÍÊAhfW?`"ÑbA–^?MÊ>ÁsŠ·?=ÛN"¥?ua—ahu>?]EF_¥¢?5Æ>?›ïž'åÚ?x–èï(&?uÎ(½ôwÎ?¤"iÔ×sŸ?™/0{:?îKò\ÜØf?´F¢›Ú?l ¦"1Õ?†¦Î,ë"?©~ÏÉï\K?³áÍ/bÍ?í')Â}ë?¤c§€Á?¡ñ1âÏcB?œ:0òj?¤ü2ˆZ?}ëf‹'?ïyN¼ëG%?~p;éC‡¶?dæt®€?X‰'ÎóèJ?Œr³Ñ©*†?{§ŒÏ`7AGN4FGL J1329.4-0530?íü·Øì7C@LçáüúÀ:¯'m-*À<P*º¾­O@§/¬@ti
à"S?ÉAV÷Þsh?Û£Ñ@yí­@ö¤^ïy ?ý¾£»º¿ï6¯õ%±j?ïæC_¿Û1W{fþ'¿ä'–NÜÝ¿ëFQˆˆÐ¿ïÿŒÝÉtSAGNbcu3FGL J1329.1-0536HE 1326-0516?êØŒU'?¸RþVÔðT?¸a"w-?µ=RºÅµÃ?°Ý›N(Ä?¢èÁ™ñ?éÌ
ÂH0é?½mQ¨'}?¿f×¥mã2?¸U¼xvª?²8ÒH¾‰?¥Ÿ|b 4ô?éíÇEpÄÜ?«•="?²È¢x­˜?´¥«Ïî?½É#ÂI]Ž?¥êõ&¿#Å?æIûmæÍ?¢»N2-Ê?ÉïÊK#{?¢'céˆ?¹Òþú'¤?'Ôö¶
¯?å&}~õ˜7?¾°Óہ?Ê\Ó!#?º;Qÿjóƒ?Á	6àf݅?°Ç´àÌýØ?âȽa·?Ë¢uf×?Ñ°(RjÂ'?ÉCQK{T?Á|ºõ£Ÿq?´ÙIP´?æK`$@á?´R1@Jæ?¼XÈ¿³?¥wÜu*\G?ȦÙo{?±L'Ò«(Ð?Ü乘½?®Q¬ß¶MH?×öõ"?±:×£\¿]?È
Â¡Æ[?£41¥&ÉAGN4FGL J1330.2-7003¿©ÉbªùÀÀ#éêÀ8±òAÑ[¨À;Ž¯­Uk@®b¬©@Ĥúö«Ã?¨VsÕå¡?ÂéËÎ|z@€èÈ«ÕÜ@ÁÝFl è?ÃÌàÃÏ£¿á§@¬m‡¿æ³˜H`¿棖b'$¿é,Ân¤ù¿ï÷`Ÿ'".AGNbcu3FGL J1330.1-7002PKS 1326-697?ïÔHÛÕÃ?¡.úþß$°?5®k˜ik?Ÿ>Áµ?"øNn¡>?"A
šª@?ï]Žyçó?š3U0!?B[ƒ†(ˆ?R國8?"»T¬	Ì?™ÍfŠ)c?ï‡ô¸p–¸?ƒ)@s?jÒ{¶Me)?r|pà.%È?‡N2îè©?€>â*bmH?ïíiç¥@?H"bÅ'œ?0É·`Ã?ñ8¦U³?`ä_E¡Ô?F`–úá1?î<âƒI	?˜§Ï¥4Ñp?…å꧔‰-?…s¦×ÿ,?¦¸]#þ%?")é![S?îe%Uuí?±eTC?c2uï؁í?ƒþp¬è
S?¨z‡- î?°ŠØnÖc?ïCÃzØR+?'£E;‰É?xÊw$"‰?€ÜŽy;"r?'Tòà,²?zð‰g?ïË(Mã?gšÁ0‹o?I>ʓ…äÔ?=hp"®?wCÿÕI?eàk,JúAGN4FGL J1330.2+7002?Ó›
÷™™@G\xB0üøÀ:S¯Ã§ŠÀ<µ"Î~}´@BÊáæ'?þ2‡V ö…?·ê"ßph?°Ý'ýuâ?ø^–ÞÔ6N@
ÂÚq{x¿çéƽ¿пÞ'</Ü¿à	¦ý…Qc¿ÚÔ¯DP¼Ü¿â{Ó {‹¿Ýx"á{°{AGNbll3FGL J1330.6+7002NVSS J133025+700141?ïúšÓ€p(?6ñyρ·k?"mÛ‰±š?Ô"ƒo¹›?@ù:~1å,?3™§»gӕ?ïÝL
k?p…ÆŸ?C²m
Cû?M!ˆ·$Œ?nÛ¶?kˆ²êij?ïË#V"¬è?eú>BƒyÇ?RC}¯3ƒî?`+ï^Ó`?uÝu=þ?]G#P"?ïÚÒðÄ?K¹†>Km?RÙàAÚÒ?1¥…½2ƒ*?kÀ½"q?I4ðùzÌ?ïöôê‰\q?AM%ÊëãÝ?10Á%gv? #¤í¸ò?K"ö,1³?={FCàà²?ï‰ü"?ŒDŠ`¦ñ?V¥Í¬2é?`ÿ5
<½?Šê…3Ió-?ŠIK‡ï¡Y?ï§õ•¡p?séN(P,ó?X[Á› Õ?_ïÃ
mú?'÷"cꤑ?pÓ㲄‡?xn?kSÌRJòå?h!öc`Û?QP›J2!?ƒRö ú:?hå|Ø)AGN4FGL J1330.3+4441?á%˜Ýâ@Q²–»˜ÇãÀ:qy¶ViÀ<©-óXQÑ@`;€^µ?þ˜DЩ*?¶ÿ{?Áh§HÙ¸™?þTuˆBYA@u>Òx³E¿ÝG"Ô@_¿ØEL»D&¿Ü⛠ÚÖ{¿àF@V1dý¿âù|"MÀ¿ïþËê'QAGNbll3FGL J1330.0+44371RXS J133021.4+444117?ïÛåÒ_çO?\Þ*"ñ;?TõžEÜsU?G²^Ä~ó?iŸ^eÍ"?VAÝقÇ?ï³/x¤½ ?€B:r¤°¢?ZZ®Ïš2J?b#ÞSuY‡?їã
7j?zX»%Ûæ?ïŠî=ŠÏý?t(ä	³?eµœŽ?eî`¦J
r?‡ÿC'Ù%?nä2ï•Ë?ï#*TÅÝ£?q1õæœ?†ÒÞª\ïÌ?cýيwt?1F==¶?hS—Ål¥×?ï¸Å‰6Ÿú?qSM<å?k&Bnkl?bj5ß{K?v(^õ­?fœ
Ø	7ª?ïår¾—?—K-zâtT?rÞdÎXŒ?xþùr'¶?˜‹¸o›ð?"Þzµ'ø%?ï5U؋i?€=^ƒæ£f?q!
G
ˆt?l[ÎÿN?•
"Ûܹ?zèKAhžY?íúÇQ7Ö?ŠQ)¤zYt?˜¡_ƒ¿?|ï»'a?¤Jº<ÁM?ƒ­(^ò=pAGN4FGL J1330.4+3157¿át[Ȏà¿@TêòRÀ;q–EQCÀ<°0Š‡@>u–8Ê@A&ÜÛ±?ÎÓʗé@K?Ò÷ ¥U@R]šåÉô@ÿTWÆ™?á拺³Å•¿»Ÿß?&l·¿éÓÛ·lé¿ßâWcJ¶¿ïÿa_3¿ÞP·þ^•7AGNbllMG2 J132953+3153?ï êœÒš?¶^KUK³?ƒKæçŒâî?yW»þöL?'Yï@²P3?¶wÕxOÄz?í]³\?ž¿`'àõ?‹ð·)û»ž?:ð?š"æÁ"´?"D´¤‡À?î
œ_5‰i?˜€rÐ-ߟ?'Š!×k6Z?Œù¥ÈÑëp?¥á)#…ƒG?"M\W®b‹?î–ÝbØN?†±Ø_?¢ú%6Љ‹?ƒAâtfÇ?–XÙés1?s¹	Yñ'?îQ70 ŒÆ?´ñèÈÓY^?˜,Ø«FM?½àµ\Ϭ?Áí#C ó?´¨‡¿+Ã`?ìýô§S¸Ü?µ
3kӓ?Ÿ:Èq×?¤Òr—
îÒ?°¨Œûèà?­úF¡‡Ì(?ìu¿:`	?¤Þ£Tº&?ŸtÑó"ö?'ãÎAþ?´tÒÛÇ5? óáµn?êR4€Ã½b?£=E1—º?»§ÌD3- ?¡õqÅØ?±Æ´ÓÏ?'¥«ÓÚÞAGN4FGL J1330.7+5200¿ãÊ¥à`@P½çXÀ:*q?|ÌÀ<€ç"øoé@–A»6Lm@'"4H?·ª4??¡±…c°?çsqF"9@ùP¢"пæ	—Xv¹›¿å	Ý.Cà*¿åC‡sý'Þ¿ç•žvx,¿å'×="
9¿ïùía—ʍAGNbcu3FGL J1330.9+520187GB 132842.6+521750?ïës*ïî?S¯jÐÔ$w?B¢t§¾?5"º@AÆ?`Jﺧú?P'½ ¼#?ïÑŒ×"Q?t¾A÷ͨ©?Jôn´,R?SÌ×¼Ækž?t<»$ŠJ0?qfɹ£†?ï¯
XÐs?qÕ6%‰¡?VÛq§}¡?ForhM'm?a;§ž†"?pð)&IªÁ?ï¶ÛPôZ?`œƒ6‰\"?lMš#ï~Â?PLý,?vkŠiS"?Yº7±3/?ïÉՃwÎ?kóV
"´?U¦ y$?EE6_?u«šïû;"?i?;del?ïqÍç÷B?Œrfü)}?[¦wRcÑi?dæ:é¬GÄ?یur2?Šs²™Š?ïb"[Áê?˜â	LÀ?dŒ ­Ï!Œ?^OËd­×§?'* wà/'?ÚÊãÔÖP?ï>é8­	?I³ʹ«?†zå\7NÑ?r­ZI?Ú°'_m?yNé/ŸªAGN4FGL J1330.7+2933?êš{ÇÕ@T@ò@úœÀ:'ßBñÀ<…0¹o¬@Êiïۛ@›Û ¥&–?ÆšÍ Y¼µ?ÑÃZб@œT\È@H‡RŽm?ìs€àæ	_¿Õ]ê–â/5¿åÑu=™¾ƒ¿ìTR½'M¿íÞæÀ=ó+?åYã¡$¨VAGNbcuFIRST J133101.8+293216?îh_|Ed?È)ÆDiß?€®zÙed?¤DMUÖó®?¥vÜ íZh?Åbllö߁?ïÂ:Åxŏ?x ¢e[?Q‰Ë¢(ª?W‹Uè?z€*MTžG?tÃÌO¨5?î–IÄÅ?™HäÆÏý?…¯."p˜?‡æÃz|×?¡37[~.n?•ò­Zab€?ïÊu^sJG?^*¿'ä§?j Áî ?RÕöÑ)?k~€ÞìšØ?Tëxˆ !?î}Ü°€Í?Àé†Û•¬>?xõÒ«7>™?‰êcÞqœ?¥z¡Æ^«?À%€LìlÐ?ïR$PÜ?—ÚyL‹ã'?fÏâDæ?s.¢íº´ñ?'áy²<‹s?– of^;œ?í³TGÍ@‡?¡Ø(pm™?m¼Ã€¢ò??œæÄ?¬"Ý"G?à=´?ï*â}t[-?'ÿۍDú˜?ˆŸ,¢í¢¨?wþ)ð£"?Œ¨3ùZ*?{ég­VñAGN4FGL J1331.0+5653?æ\h2ÃT@M´k&¿‡jÀ;Zw'ÔáÀ<ïcáPèP@ ùŸõÿ 1?öûUvT?ØB·ÀK41?ÒFŠþÌ#?õb¥ç…¶?øj¶ü¿â°›ÿ$Ô¿ê[a .Q¿çp5½Q.Ç?ªÁdÂUD¿ßZ_U¿ÚƒT]ÐAGNbll3FGL J1330.4+5641RX J1331.0+5655?ïÇ\]<û?€Ó¤ðIZ?H œ¯rh?D
óbñu?yP6AC?ÜÛűx$?ïy»‹d€;?'Knú¿?i=½ƒ	\?uªâ™¡'?‹O
´gˆø?ŠN=V ì6?î¢Z÷ƒ•Ý?"ƒ%ÅԎw?v¼Z1Lp?xHp}º@?£ÙH
—?"i"ñ'?ïíë€l!?}-4|'nž?q9§¬ÜáP?`"úû¼ ?›3ب*߅?zdó;JÕ£?ïi—"rè?WÐM?5æ?U
hæŽ?LIìpÝC"?'|¼¯—^‹?­Á«bm?îuÂÌÃ?­ '·F5–?x'D+Ù?‰
Zړ ?¥"Š¾Ùm?«"a8[?í¼ Žø£7? Z݂b×w?z c˹?yï²û¡hÉ?°põIÑVá?Ÿ'(Xð?ímÁøÄÞ?™*~(°ës?{Ð-Ò8®?t
v@Æ-?²Ôñ#7Jl?˜hC?­°vAGN4FGL J1331.2-1325¿î½š8a+¥@H'M3H,À9™X¸'úÀ;ŽŒ3‰M@4@#‡@èŠÛ´ï?Ã>êáà°/?Í&ö9ÔA@ PxË@4j­óò¿ç¬h=Öû$?À‰ßgY+¿æ ¤_ñ,S¿ë`ö í¦¿ã°W¡&«»¿ïÿþøþ"AGNbll3FGL J1331.1-1328PMN J1331-1326?ïÜ?aûÙ¼?d<ñ_?¶è?LˆÖ+?Aß7p©òõ?lº{çWµ?b!HõhS?ïžÎ®"´?j·t?d¡òXP?hä,"'c?ƒ$Õˀ÷?y ýîR?ígªfE"D? ªSéö¤?"¼_s+fx?Òä¯ï?¯')䥽‡?kîÿR?í~š!©Èç?ˆ&ƃ֐z?‹–Ü-›wH?mY…<He^?°˜SlVb?…šK»ÿÆ?ïœÚïØÉ
?…ÿd"lGÁ?\áçL¾N?X…˜àÕûò?…-ßD¥?"Ò©8P±ý?î»@0‹}?¡ÑÉA+ã?zwK§w?ƒaVÉpºé?¡3íIB?ûÙ¿Ib'?ë¿ä†ýµ£?§ç™‰Þ?¤†r
ä~?›4Xÿ?·¸˜àª?£•Ú~Xxý?é*·G:¸I?£˜çÁ:Š?£==Š:†-?‹ªÊ"Î$?ƅӀ½w?¡²‡ßÚ\AGN4FGL J1331.6+1711¿èõ½B¯ì±@SEbàŸèÀ:@óÖ&À<ptšÐ$@-…àT>@Á]}‰˜›?¹<ÀO»Õ?Æí|Õ¡?Âi;,ü¸@R:«økâ¿Ý«$[¾¿æ1L©%þ—¿áëâ—°¿åTÍ·®X¿åÚ;€ÎÜ¿Òg'áC§JAGNbll3FGL J1331.5+1711TXS 1329+174?ﲧH?-?v¨%dDÎh?Rބ<°ì?@ÓR›)ì?€ú]`Ѥ"?uò2aüõ4?ï͚ôÒ>@?uŠ˜ÿþ˜ñ?KUÑmK1ß?T[#j§äl?uÇËI¬©¼?rªv€?ïEå¦Ò+?…
íûÜßÞ?i)Šõà??dvù3Ř¾?"ÍYÛ+?"-¼Ù<*S?12°Š?chn¾£Ž?kö®m¸?P&vGW?€];/Mm?^»qÿKx?ï4(¸IÌÁ?‹×•·§"?hxà$çË?ZZ7ŒéÇ×?–kÌñy™8?Š2Vßø³?ïfûp½ò?"oWž-š?]iÇ	t'?fg¨ùaÂ?'Iõdh?'«ú°ô7?î[EhÈt?—ÇÌHG¶[?{ Ù+eÊ?vªD¡ïxN?¦Ú"Áø?•|ø§…»L?îèãѬ'?ƒ?ð9õ(e?"ü#¿‡EØ?o)Dï¬A?˜et¶fâ?€(Œ"zÉAGN4FGL J1331.7-0343?¢?UKÿ
v@LÓ;÷'À:]òœj.rÀ<Õ¤ãc@¾k[m¹í?ùæ(S`'?ì1d™ˆ?æB^
ÒQ?þÛÐ@Ô@T@¹Ù€?åðg¦ØF~¿çQHÇïî:¿ã&ØaU…n¿ïÿèã«6¿¸š¬È®¿î:
BâMAGNfsrqPKS 1328-034?ï^ß"S¬?&¸´R—?PJßâŽÉ¤?Rí
©³?ŠìHJîý?‹þßÙä?þìüå?'Q±Ü-(\?h
œúºÚQ?}6¦Í
< ?…˜ô4+?ˆÑùä0a_?ëÌ7Ô,½x?¨?Kœé?¢©îÏV?›7†îµï?¸Wle"^•?£‹!–/?ï(s-8N?ˆ6ÉíS¾??Á߆÷r?@*臐'?šr'ÕÁNP?ˆ¡iõü—?ïÄCÍpr?«èÊë\k!?c–ë¥é%Î?eÌúiE|?4šÕ
?«Ãktú;?îÙ8¤rvÑ?¨:¡M+?{Ò(v¬²¹?'}Ù%žì?äaKÆé8?¡GÕÎöj!?é"ìl¶rÔ?®U½üÄD?©y_Qâ/?ìÍ»b«Â?ÃR5ö©b?©¯`	½ßm?îSIoü?£3K½è#?4®Ìß©¸?Pç6á?ª¢i²,TË?£40s
EAGN4FGL J1331.7-0647?ïÿûäE@KY†üÞãPÀ;ÂHåL À<žw{@áqF>RÌ?ü™ƒyœ¤?Ïm"ÝzÅ?ÓW,u©Ð@»
,©¬@6ŒØ–¸¿Ë»±\"?ïø €´ã¿ËÊ+éÔ¿à›¾'1H"¿æW9''¦¹¿á¹
"BËAGNbcuNVSS J133146-064632?xÐ\‹?‡‡xƒÙ?d]ôü»'Æ?m]¿£~Ô?"}¤€nÀ?ƒÃ̼Ä?ïeM­e†ö?Ž9½œöHÜ?up‰ãív?~V?¦­Ú?‹ôO¤IÚ?ƒ–I	_?îhïhê5z?œ&«qzš?µ«ª¤>?dÈ›‹?¡3š¢ˆJ?"`¤¬?íom‡S,?†%C¬3Ay? \B—œlÇ?}Qèåcö?¦ÌƏî`u?€ÎCvJª¶?ï[_چç?½"Á¾)[?vœp1?v@uHæ&?Ù;-5-?ŠÜÎ=3hí?î°ÃÊp?¨5}ŒÞûB?ŽˆÞ`WŠ?"YJd¡A
?¦Òí''*?¡I•$ˆÙ*?íð©"Y|¯?œêLAˆG?ŽSìQ§†?y .Gæ?©p'¿SË+?˜o­js"?êÿ·ªÉI?ŸÿI} µ?ªKv8%[?"°sÿã¤?ºÜ‡ŒÉ?˜±ŠÒjAGN4FGL J1332.0-0509?ãJhH`8q@Läy'¼VÀ8¯ ÄÀ;'ŒÂÂ#@	"'›Ø@&Ð& û? Áø»ñÚ?Å[ôœî¹@ †/Y‰ß@»û¢£-—¿ÓéŒÁDŽ¿á•"Ì'úò¿ç–ªÁµ£¿êqü!#;C¿èÜ"¤?¿ïÿ±Æ·	AGNfsrq3FGL J1332.0-0508PKS 1329-049?ï3WŒ?$>?¦q–>r
ò?‰w+³÷?™"Xþ¾?Š¥Ëb0Ð?•Ž´.Š?ï°/D¦›?ƒ\ʛ™?ZÀ;Y-?j­¦»ÓB?€œ8ŠÖø;?€•æK˜î›?îŸ'OÐ!ì?žêـ£ú?'7̓úšÒ?'Ôð˜ë,?šãIlÙ½¹?–uC)ôÎ?ïðˆ$¹?IEZŸ9Ñ?C-}íuYE?5ÛVrfp–?V<0ה+?C>"¡UU?îÞ§äÂ-?¤ƒóHšJ/?'ÛŠ×iEÚ?"ô"Àãú*?'Ox¦>tƒ?›<»Bî?ï";I¾K?ž\ËQ{ü?pÈ\%–M?v(Å(æ?˜s|{0
?šg<V/3?íÜ%*
á?¤é9îLõ?šOG.ö_.?™Aµˆá±#?¥	ÌouR? }ª­k-?ïÐxëú¤?fž ›iÉ
?\€"&ËkX?QÞÓª‹?p£e"¦í?cSð>UIAGN4FGL J1332.2+4722¿í•Ò¢y½@Q篷éÀ:]N[­¥ÀÀ<tZ5Ö{¢@E–hâ˜@Å1Àll:?À±µY¾D?²†¯‡µ#?ïOo^²'å@
$¤¥p;?ï¿àÀŸ—à¿ãiWaæ¤å¿é-h]â^Y¿æ°<g™í¿ëñ§½s¾i¿ïí…èÜÎAGNfsrq3FGL J1331.8+4718B3 1330+476?ïè؂ÒF£?c};®Æ–A?G7"ä14?A*õQ2¶q?ac/jrÚÔ?aáz‹cÚF?ïÐ6U@h?vÄÂØþB?IN5íÔð?Tqå!¹­p?t»±æð?s\˜ˆªº?ï´)?"j†?tç¹vÅ8?\`:ô(?] êó1È?~ÓQÅFP?sE'SM?ᅤx>C÷?\§#þ‰s·?l½·¾M?PƒU‰?r2åA¥?T>éE?ïÕ.ð×e?kïÚQÈZ.?[AT:j66?aÊ®3r?m1OÑwS?b®V·9¼?ïvŒ'×q?1óB,u?]›"±"Gä?f|&>ʕa?Ž©l0»ðÃ?‹ØóMtdò?ï~›)DO™?}ê¬ãΞ?fÃÒr"D?hÖÐCV?Š¨A¿Ð?y¨ge[xÈ?ï)Y‹ó¤ä?å÷I"Ϥ?ˆŠ|>kªÜ?s¯sƒy? ȸ?tµ$›0¹AGN4FGL J1332.6-1256¿ãnjõI÷@HYµà÷üüÀ8ݜþ¨èÀ;.
—~6@†/8§¼G@8"üS£? øÙßɘ?ÀÄEª.<S@ØFèòA@õxèt¿ÕH­ûŸH¿â׌™¿æ=é¿æЖP8ýx¿éL!`ø¾B¿ì
Gahz¾AGNfsrq3FGL J1332.6-1256PMN J1332-1256?ïÒVvÚ&ý?j+ë,¿"Á?ej¡´p4›?`ôT—±3?h>çZv?`s»c@à§?ï¢gᐩ0?"N jrÖ?b¢Zq´L÷?n›<2hŽ†?'½pü¨ðÂ?~n¸Ìè	?ï(ij·;?"åÆs
qp?Ó‹$XF`?'rKèYòÅ?†]"Ë?…7_ᾫµ?ïJMЇ0O?|.¦x{š?rðvŽì[L?a,¦ò]®?'ú(J'øF?wç	çšæn?ïŠæ†dç?"‹Í­1!?xç7ÿ4s?wyu
P|?€ÒÂfã«?zŽ€K•ÛÄ?îÕãïªb?¡]WM]šª?x¢þ¿…‰?‡¯ð\ij?ŸAÙTŸ³r?žZSŠKý?î¨ýp^a?›Ö6Q!?˜¯²›Õ?•Ù6E?ü?'0´Kù2?¡Ã?ÍxÙ?íž8ËV2Å?œÚîèDfP?Ü€ïkw?€8GY"Ðe?­®3F¸Òî?š
C¿°J.AGN4FGL J1333.0-6626?æl.Šé
ÜÀ9æRlÀ9åüágŽ…À;|Ëëü<ý@<r‰à>@9Eßaô?Б} <5?Òb÷{Ìÿø@3.`e›e@QøV¾R·¿· o Ê$ý?ëñ_ˆ{º¿çGQÞD‰¿è³¾smµæ¿ïÿ틉5ž¿ä9óEAGNbcuAT20G J133254-662826?âôÍdwMê?ÂÖ	ÅnÆ?'·Årž*?‡îhƒ+ˆ?Ù9»°è?³_M]?çGúÕô"»?ÂpuHy?‹fšÛç["?‰Æ@óc…#?ДÕ}S?ÁÐöŠîd?æ\¥6I­?°sՇ•çÝ?¤m—S¶cé?"',kWŒ»?ÑI"Ë#I?¯PùB¦·?ê¿á""Ï°?˜t@pgÚ?¡·¶þñÈ?~¾ËáÏ7?À'Œ/ßÒÊ?–¯î´lób?Óë!Úxåx?¿?ðÐ>‹?œBó÷\c?–¨l"ÞW¬?å(Ws?£ë?À:Ù©ÃÍ?ÝtTP9S^?É}ƃ¡N‰?œAZõ6Pß?¢é.ßêË`?àcËhz?ɀ(#µ'È?Ùfs~Ÿ9¹?¶—}P0ñš?±q?&•ó?›ÖUxÀÇ?á¥XÙNÕ?¶Eâ¬?á?åϦ"Ó"?¨×y¯0"#?­l—§ØÊÓ?"{÷4cæ®?гã±Q?¨z
m8MIXED4FGL J1333.2+2725?ëϾÕ@T,¯¢ðZqÀ9åkÅKÀ<ƒˆ×@yÄqßk`@/${	‹š?³5ëId¢í?­/)ä*—?öôLfàà@
"ÞCÿ ÐU ùè¿ãX˜GŠM¿äH3
‡¶¿äbYDzä¿ç#…uö&b¿æz˜í¢/jAGNfsrq3FGL J1332.8+2723MG2 J133305+2725?ïÑÊøâ)€?£	ÃˌÔç?4>@"Œï?3\ûQ]™À?uÖ¢-¥ÌK?£é]§%?ïÏM(/|£?uÀ«$?IÝÑh¯ø?UíéÊ­çp?u5ð¡nI?rqtñq-?ﮛÉʎÚ?U œ‰§?T'ñ)€?`èSÔþöq?È¯qE?~‡êƒ5»ä?ïÖ¢ê³?Qéí|GÈ?eˆrT,9[?HÚ$Gã?cÕ|ßÿ£r?EqËôނc?ïÌ%ҙâ·?'!M×sÔ?E³Ð
¦u?<yj¼7ÿ›?wLÀS;ï?åŽƒF·?ïiqÌS³º?"Ö¨Gü%Ò?[*ÕÉz?h€o6u?'Õ³',?"«
ôÛ?ïsgsà**?†ý0Þ=dD?]Á·Ë«àÿ?S 5Ÿ Ñ?mìv×=?†¿$•°?ï"*Ÿd?p¬1r¥ü4?|6º¯Ù?eÍ#pZΈ?zH0ŽœÊ(?dBÖR«HAAGN4FGL J1333.7+5056?֛F‡@P7Ù+à‹À9QpXW¯êÀ<&€Aÿ@Ž5deÛ&@oZµ?©Šނ›•?¶ðBrÁ=¢@äLæb @QúÝv?ßÝE€gÄ_¿âïÕ¿ä•`ß鵿äl¥¡·¿éJS
iŽ¿ïüÒf(SAGNfsrq3FGL J1333.7+5057CLASS J1333+5057?ïí&=κ?R¾ì¿"k˜?D§b?9šBœäö?[¨€»ý?O#é½þ4?ïÙ(Mëµ?pc^ەÛ?D(³&ȯ?MjßÊm»9?pëÕz=,_?l-·yx™É?ﲅOy~¶?r£µýWK?e©[ŸAÃ?igj±E{?{誓Yì?iöj›Õ3?ïöi;,ü¸?5ºË·?9ƒöÎN(²?"g»z1"?I™æéR;?0D†-^?ïØKS™ß?n`)ªV&é?P9 Û."ú?Ex ÍOÚ?o—ÛðÖh>?lŠQ¯¢}ï?ï"÷")JÛ?‡Sg½օ?Yμ;ß?pB¹á'?½?‡ˆC^c2‹?"óˆÊÕ«â?ïir|õ%?ƒJ¨Ž_ÄÙ?w²Óþê?y+Ž-ê›Ø?‰ÊX/?Sj?yÍƏ€?ïç7RbC?SZÐ*WEý?Pǂ9óm(?@°5mexi?`dìâÎs?N³|ê[ÌAGN4FGL J1334.1-3521?¸Ú°æl@:´óý">6À;†qž¨ÍÀ<µ—îáË@",Ò£üI?û e›eK´?ÇÜìš"ì?{øVñÜÚ??¸=¾./?üKÛÙ=§¿îGø½Ÿ¤?¬ÜUÖÌ?ïçB.x¹O¿º‰#ªª
/¿ê<Œ¾÷Y?Ï1úcˆænAGNbcuPKS 1331-350?ïY¶09iê?¥¥{Ŭ‡?T˜I[íR[?V'†ZµÃ?"µg·f?¥]lâþÔ?ï°XŠ°—?ª±ÜëÚ­?Yãéq}"?bd'+aYÄ?€­y³:Ί?|¿šqr>z?îût$6}?UýrÝ?u[þÀÿ%ó?{{²y÷ö?›:{Äæ?Œô+e¨^*?îÆ^d	e?:_cq J?l?#=\*ó?`(õ¸ðt6?¡Ö'‰Cъ?€^{Må¤R?ï
ÝÞuŸ?›ãížÖ#Ë?_¡ð'·?T­X¼"fM?œe…J?.ã?›‰.§Cï?ï9|þ$Õð?˜õ2)o{h?gCl°ê-…?tðÌç¼?•çò©;‰T?–¢×vml?î>ø•ÊÏi?–¿Ë
ƒA?||\ÅÇU°?|Òv·nÐ?¨€ë
ƺ?"SJ£ê?ìü}ÆC?že=\Üî¼?}›Ï+ZL?|öàÁQ;­?¶BWÕMd?Ñ¢­Ð™AGN4FGL J1334.5+5634¿ÔŸ/z0@MÈà"'À;J&˜=™À<¾2‰}Ã@ÅSÅ$ù@÷çbzH›?ÃJÕ¦»?¿ b3Ѿ¤?ܦÆ0<‰@£úü5>¿î3(¶ØnÁ?ï®þ`¿¿çêUp
¿ã½¢W®<¿¿êøýâïN?Üá­å+}AGNfsrqTXS 1332+567?ï¤äl{©?{tO‹í?güˆ?Z´BÀ…ž?4Çب?}?w橗Œ!?ïÍÈÇüÐÃ?r"cPé›Ê?Hø`Ï¥¦?QòÜ{‡?uüéÁ³?oæ8–©?îíUtaâÚ?1ªb ¦?w}µº]Ï?vj4£ÇÚ?œuä4|ÇA?ƒa®B$?ï´å`-?`ìÜS©Ó?k§ G]?R›·¿<?w¹€ÃA\?Z²p¶ .?ïaÎ.Õ3?'.¤0µû0?|`§é?ª?t­<ÒIá?•[œ?¢±?ˆê:j
ë?ï^‰Üžb<?'ßGÀâGƒ?_{ɘ›‡ý?eˆ"!¦¥?'7К;õ?›8±ö}b?íôÈ:0?›9-"Ï?€ìýbw‰›?z®[î>º?¬ƒP,W›?™Ý=(?ïd^ ?'ÊÀþ''?… %#ö³?tmÿšW—?"ãlÌ\Ÿ?{ìT-}~AGN4FGL J1335.3-2949?ïý9P'Ë@@
=¢ø½ìÀ:_ס<%JÀ<i'Où<—@ÏÄùÛ?ÿ@Íù¦J?º[ˆ'ßf?›'ù†-?átþªëQ@é
<€?î&üX«'À?ÓsºÂ‰'¿âþiȶe¿Òi7;«|Æ¿ån)¾ÀD©¿æ¾[ÏßAGNbll3FGL J1335.4-29491ES 1332-295?ïå³±ói?SÉ	ÔT(?C³",Îà˜?5X"Òîç¯?e`>,š@?P±å€ÐÝl?ïÚV'î‡]?rÒØ¡~*?Hl—­ù?SÉe§©Ç?oŽWÍV÷?mÖa¦,1ß?ïE>'P¿?€->Œ\?aùˆ3—€?j"·#1!O?‡°NFFü¸?|‹‹ªÒ?ï||–DÆ?hÃN Î?tؔP	zÏ?Vj™`j¢+?†t[éq?béæ ¡ãM?ïÕ¸ÈÂI?eÚÈx«=«?QóßP×	Ç?GRòÂÎ_M?p§_v])?b×2mÚ?ï¡[.qNï?†[û"´?VU'qóå?c'ŽžMj?"Þ'&ÂSÐ?'·-Ýj #?ïB91¾­¿?ƒ'Y6+¥ë?jšˆdº€?q\Ôžõå?"eˆÀºb?QÖ|šû"?îÁ~8âl?L܍Æ7î?‰bî?kÙK?rMþo—÷ˆ?›+Ù-ÅØ?zeõ[ðïQAGN4FGL J1336.2+2320¿ä܇ã8Éö@SÌs-õÑÀ;:ØC""À<ºoª²Æ'@½mç94ª?û.ʸöV3?ÓÖBAn	s?ͽ—»!ú?÷إ̭Ã@ۅ9D†?ë·Ç'
0Û¿ì=¥b$¸F¿ÍºÞæ¿Ç°j–vÏj¿ç€…@dž¿ïÿÀªšëAGNbll2MASS J13361219+2319581?ïÚ4u'?igíoo¨?KTJdέ|??…
C|?nöl"$'?g,Ö¢PZ?ï˶ù77?}BXävx_?I²ë 1:?R<ÀOcß?wìô~zV?{'ìw9?ï]ڄ×{ä?…'Å[V²?cæ±ô[…?ea`¾îÕ?'ÇÙ,ˆrv?"¸ŒTàÍ£?ïZ›—u§ø?nƒCϊ,Ä?n?¾´>·$?RêhvÞo?ä•9M"?l«~‹-À?ï¥tG"X?‹BiÌôÑ?caµ?Ó?‡jZ»7!?â•¹H·-?{D÷Wš-¯?ïUE#BÑ?—³þàöC?\}s¢Qâ•?iÀeÃû®<?""b'Ö¹?–b¾±Ä?îÜJ™´Ð	?SiÖÕ±š?n®]IQð?l°zŸ(? PpŽfa?ª•'`?îiUþ~"?Š–efôò)?wý›"ó&#?i]ƒ¶|Ø?¦jì¦êŒ'?‰Óyœö†µAGN4FGL J1336.2+2053¿æ"¼ÝìYÛ@SÿëJÀ:ã
æãÏHÀ<•¬Þð¼@¢3k½=c?þԓj«p?ÍÙ_m=p?´".›säS?ê–
ΐl@,.Œ…_?ﺌޠ3è¿äÜÃàj
¿á‡—¾V迼e®Ûu1/¿áƒ"Ê/c›¿ç×_f˜AGNbcuNVSS J133612+205102?ïá`«ø}?YS±Iäl?4Ǫ‹ä#–?"žË'ä?l^{yà¤?Xým¦!?ï×â%é7€?q®JI²øý?AÖÓ¿†¯?JtÛ}d×?qÔª¿>>?pDÏ«5
Á?ï‰T‡8:{?r™ßEe‡?\TbUæ?[J"ᙚ?Š*S»"êX?p\5{Þ?ï'=r"àX?iy‰èŨ?cJBwSˆ?GE–­%®?Šž½+uù?g–4å°ã~?ïÍ[*H(
?eœœÒó?="ŒÍ"Êv?+ϲﮑg?w€BZK\?dÉd¯wgn?ïˆ7ªn܊?‰òƒ+Y?QҞ|'"ã?Y†'¥‰)p?‹·Á"Vá?ˆÖ}АPÆ?ïìë$i?"üô7ôv?et0HÞa?\:à"Up?š"Ü'Ø?ƒ´8¨|YB?î !ë(?†ÆÛR=èØ?vL¼×™Qô?e:ün½°J?£66Sì>Â?…±ø<AGN4FGL J1337.4+5502¿êo<dùîˆ@Nm©CZÈ£À:ôå‹àssÀ<¤ÝŸ'ç¦@_o̵@Æ"ï¾?ÃãŽe?•g³™ú"?Ñrd`ý›Í@
Íî¿›\¡õ*0¿æp@o[Øn¿î8¯6Y¿ÍÈ#à{Ö¿àAœbKό¿ïí…>˜ÂAGNfsrqS4 1335+55?ï›…ÏÀÑ?±1VgDý?FÉ"¹"CË?Zšœüãˆ?‡³Œp!ŒS?±ysݓ?ïÜ{Íð?mΤ™€±?BCS.ûâ!?K ÂØ»¼?ohtG¤&?ipz?î´æ:d1?œÏ§îRá?\T':ñ?g‹{3&ñ?£Ñ9Á]Q?œ…µŽ§?ïõWµ?;'J҂‹?3	¡Zvšê?!¿K)"?PŽ™ÍÿL[?7!œ®ýí?ïñ‹»Š…*?dÁü݉O?=q—˜¹x?Lx¥»Ez?UŒ"ƨR?bÆæ%ÙÒ?گŽx?…×à'ý²ä?P¹^ÈB½?[×;Ào?‡†tŒÈ:?"<Š134#?îrkáê/"?ŸŽõ»S^¿?bBãaß" ?iÝ¿×Ò‹?§µ¨Ád@?Ÿ˜¯Í¡7?ï×YÝäC®?`;q^©»ö?WüV£f~?PÄFjÃ?l§Ú¡äþ/?Y!O ôoAGN4FGL J1337.5-7802¿éQÉ5`"À.ÉÄüó0À:¾eò£ +À<jGW­eÿ@l/µÐ1@¬¸?wT?ÈÍvÀіá?¸]/ÛåÄ?ñtVéò?é&ƒZ?î48Ùeb¿éÄ×5›J¿å"åÕ²O¿ÐÓDá"é¿æŽBM'j¿ïÿ«Ÿ7=AGNbcuRX J1338.2-7801?ïœi©Ö—k?"iìýF?Iú}q§§?Q–!ÁN?‡Eí{í,?ƒ²àþ`*Q?ýžs?«r¿Vã?‰ÍÓ£?'Q֖¸?¡ŠÑ9b?§m_«–",?ï§Ìüâ-?(Q½=áÙ?s"3ðä)n?y'ã#üa?™Iù^«P?Š^èú?è×I5'?¢6-Á1ͨ?«Îgêeˆ?Žˆ±Sšgè?ÆÉῼÞ?Ÿ¹£'Ú?ïw7Û?'ÕÖs£?[6SÐiëÓ?ZGøOÒ<?š½³ÜSî?'v›s֔á?ëpœ4Ôs	?ÁÊ?¶K?©b•³qa5?´¦¡
Ü?·ÉÓ~ÇÐ?»'‰bb?îRÆ´ôƒ?–Ö­(ö!
?€ÔµP8ºw?'Èö=†`¾?¦©V=2í;?"¥‹äQ9?à+Õً?­žÿðFÁ´?»5g@ 6?£/+ïJÁ?ØÚü:?¯Rø²o-©AGN4FGL J1337.6-1257?íj'ê2kì@H0W\gÓÀ8¼^ÑF¯À; *o?Rü@€|»@p…ÔÀ·?ªâ¹âÔú?Á·œäÒ¨@÷x‰|ì@;ñ®ƒ‹?ì赖Ob>¿ßI¼±K½¿åºß.Ï d¿æÉë	ζ¿çüQ¿æ4}¿ëãú !°AGNfsrq3FGL J1337.6-1257PKS 1335-127?ïÓÀ±Wó©?ˆ#˜uþu?\3S¯I˜?t2æÀìR?n%¤æe
'?}׿é?A¢^?…×ݳ¿?háç'Öì?ś7Ìï¸?…5Ç£rT?€@õU¼|?﭅ëxÓ?~Ìl1Xöè?co¥¦'K?m
ÿ›4?…7qbA3?y?ÿêœnž?ï ȟÁ{á?ul÷
3ãf?…÷0áQó?h(
µ	's?ë^ö?ä?mja‰¼
®?ïÇùÞþ¨'?r¤¿P"5?W Æ9–?QÈ
çC?v;cºù\?p"º‰Š¢?î¨!–?¢ÍXÅ¿?€‡gîFß(?‰ž9–˜–?¡\ª®\?žöte`'?ï}â÷fK?ˆåS[­3?i€qFj¥Â?ujùÏl?Š'_²›‡Ö?…¥MEÇÏ&?í¶ã!U˜Á?'cî'xA?~÷2Ð,–?"æT»Ì§ì?¥ÒRNª¨£?‰Ü¸Ì;Œ±AGN4FGL J1337.9-1956¿î}¿®2E@DÌsWæpãÀ:ó/p0ÄÀ<;+äŠX´@Œ·ÔCé@¶5¾þ­ð?̇À键£?¢(^Etm?ÕØÙJ‰'@
lš­•Ïà?튌Jü}•¿é¨USïk]¿çN'ÿú ÿÝEâb`Gh¿åšVÞ3&ž¿ðAGNbcuPMN J1337-1958?ïó¬Ü±50?Kýí—?ì?.îóÐÖ? ÊÍKIŽ?TȂTtq¥?I_Iœ.¢V?ïÆ*¬QO?w¾›l9²|?LšÙª¦Læ?RÒv¯ß¬#?yWN"çCù?u/¿­Iåª?ïˆÂ"9³U?¬Ã=:Ò?TãŠõY?BÏeKTDÈ?‹2úf(¢?güõÐü?ÒFß8?cdz'ù×?Lyîô¯(?1¢=¾0?…Ölw'JÚ?bÑUáö
?ïæn‰P?aéÌ?8¥PÜ íÄ?/¬Fë¯?f}NCáªu?`/~=Šµ?ïk%^D•?'"áQqÀ??UõFו~³?`˜þOÞ?';ÿÁˆúO?¸'ªƒÕ?î÷§<š™?™,͘˜ ?a¶HBŽ@Ý?WV$yÊg?žÔSÌ'WÕ?Žý­l·]?îÆÝÍ%7G?ƒÖ~å(ÝF?e¿/®uw?RŸMËØ` ?¢609iê;?ƒP›ûÕîAGN4FGL J1338.0+6534¿ã"…;	@In¤"‰—ÄÀ:d¸ÄL0À<…Ö9ïæ@´`àÀu@!‹…ÚŸô?ã%Éé±?¿6Ü
,~¹?øôèû¼¾@
)Öð? °XÍÌ|¿æY	áÖZ¿æºl­¨DW¿ê"öÕ®¿ïÿµÝœþ©¿ïÿ‹Á>ÏAGNfsrq3FGL J1338.9+653287GB 133543.8+654752?ïò6‡aÄÒ?Ig;*YÁÙ?C«á 'óh?5Qûi"é?Q½ÔIÄs?CR>T²?ï¨ç:"Ùõ?Ý‰oO?a´ˆÅÿ?iÆ\ù³¾<?Y_÷:ú?{#"¶b£ö?＀!߉ú?f·ˆn®Fj?ZÕVó£?N!	4ìè?{
™U`ãz?dS7ÇVë?ïŒ7Uy%¨?fF;½_5^?~
N²GÇ?^€ç¤r?{×	ÜI?]NZMÖ?ïÝ-%/Âï?cG|é")‰?Y€¢4šQÕ?Q?¬ó$?f‰¦Ñ O?\q"òK?îî2֟'
?œŒ¡‹ø?u`Ûòo?€öcPÅÐ?œán)Yw?–þWÂ^ê?ï'òòŒ‹$?z«fÏ°•~?cÔÏâܵ?Xµôè š'?ŠNªw?xr·?åMÃ?îÛÌ3l?ˆlœrû¢?—t:Iü?€
©bÂF?–dF
›î?€:{Q´"AGN4FGL J1338.9+1153¿àô#P<-ƒ@QÈ\|ؙÀ:»WYƒ)À<XEq
‰@òv`¯m@@uá;ÚÂ?³AwïzÌ¥¿–gڄÆMØ?䆼²£UÛ@ûû!ÉÔJ¿æÁáìï'¿Òƒ`½Z¿æy¶Vi¿Ýá‹5RÈ$¿Î†Ï'y꨿è'?
äAGNbll3FGL J1339.0+1153SDSS J133859.05+115316.7?ïÉs]è
?­ß°9¥/}?H.QîâP?yÜ¡
þ±¦?x@"'_Í?ª±ÆG]ÈÄ?ïæmÇY?p\D´BòÙ?4·ö%j(?C]ô|¦ì?ggõŽ‹>O?n	ûL(Û?ï§õmæô|?|ìv®X¨™?O¶ü@Àd›?=,¯únü?"4¸}??|½(Yª?ïâޕˆN)?J	
¼Nùþ?<ã×ÌÖã?$6û&±D?i"ï¿Hº?Hã÷*K¿?ïÝr׍ðï?v]Ú×¢¢?C,«É§)Ç?RA‰øÔ?mÁý†> 4?r{h#¨mF?ï§ûÞŠÍ?"ïhãVA¤?Hþæ2Æ<b?TÞ	½Cn÷?"qP'K?ƒÄXN""s?ïZ`¾j?ˆ1ێ>n;?X.uG£'O?W·îBb+?"1Š¬?‡Âр£™ò?ï«¿gDÄ?iÖÇÐÎ4?U1둫?E{ö7'?¦?'œ
Î?gñÀ‰^ï=AGN4FGL J1339.0-2400¿ê–NÃT@BËw[0À9përáÀ</;©#z@ÐÃ7LÈ[@÷3¨£ù?°k̬Ái—?®ý&¾%.?ýt,!Æú%@tn}·÷?äuÞÿT^¿âJiæM§S¿ãqø -à¿ãô±œ]™¿è~¶ôô3C¿çR¾éµ;AGNbcu3FGL J1338.6-2403PKS 1336-237?ïìfîÕõ?SX¬™Q?:Vt<™?,gŸ¿¹?`V¦¨gg?Q4¿@šik?ïÔó¨¿ãl?s_ô²óöp?Lpˆ/Zu?W+–7`©?qø·õýÙ?nè?ïÀE"M™*?f֐V?UYòç;?EÎ79¶Þ?z†¹MÚ'?dؚËE?ïÆÐËxӕ?Uªßi‡=?aÜ;ºt:O?AýÌ|£r>?s©|O®¬b?QªGU˜ÒŽ?ïÎ?cR?kOõ•©¯?Qދ5²¥=?Gƒå'Ém?t€½akF?h»õE?ï'"dXð?‰»ú<xˆ?[¶HõéÛä?f5³y•F?Œ»…?†ÞÅÝ?AÒ?ïŽ='Ý'Ã?v)æ.xÞk?bԜõM°F?]¾3ÑA'N?‡»tÇC8?rãùDÌÑ?ïeŠÊã'`?v³d'ñö?xär…v×?`[QÓþ4?Š+Eƒ5â¸?qnôáD¼AGN4FGL J1339.1-2620¿Õ'ƹå@A¨hۋ¬qÀ:u\€3—À<o'OÐ!ì@_y';|-@RÑ84$?€*ä ©?¹LuN‹©A?öÈÝ•.@
'áG®{?ïJùùUÁÓ¿å½K_¤Ö9¿ápXô©¿âÙs8ÜÀ`¿äÅ"}c¿æŠD'HAGNfsrqPKS 1336-260?ïï‹DL$?T¨X¤0÷D?4u(י+¾?-ß«osŠ?[̬»ê7P?Q«º‰£_E?ïàtOï<Ê?k5Es‡û!?=e£+ž05?FòÞúX
Ð?kÞû<G?g¬ëÚ{Ûq?ï…&"²?g¤0ǁ2?Ro?Ė¾?@Ø}Gô¯?z!LÂ&‡?ffÂ[9?ïÃç–&Èl?TuaOW[?SùU¶$ȗ?0­ Øvå{?y
ߎàËå?T2˜/l?ïå0"=+|?[Hš—&<ø?@‰›e/?0§(H¬•Â?f­ò\M9?Xöô€RpD?ï£Õ0¸Hu?"zëÖ_k?Q?ìò4¤ó?]­6çÃ'B?"â¶)Xz&?'}i¬ÓÈi?ï–êñ·#)?uøe« AÎ?]ƒÞÆCK§?V;">·§?†"Ç© ˜~?twu¢¯p?ïKµwú?tö%áÿ?jÐÏì2ÿ?NW£êäÍ?"3ÏUâ6v?tDÜD6UEAGN4FGL J1339.9-0138?ïF\Np·‰@Mzj~ùÛ#À;=[XkÀ<ÜãèrDÁ@‹‹ØeÝ@ñ·D¥?їÆÆ"Ž ?åÀGƒLP;@Qͽ"©@ ß=è˜Û?ïõêgèF¦?ÜWžbP2¿âG~>œ¿å @LÜ'¿ïÿ¶>@£?ë\e[¤k…AGNfsrq3FGL J1339.8-0133PKS 1337-013?ïQGEcâ?¢‹%`ØJ?"wÒB¯1n?ž|»¹ëN?"<	žùН?"@>"iP?îP	þº
`?¬íÀH–-?›:F*SM?¥|14ó€*?šÄz8¦?—MÁq't?éš"£n¿?¬É[u"ø<?¾h‹;ªG‰?§]˜ùƒ?´Æ_«[ÿ?Ÿ€Š?îƜüœë€?…§4x1ÞØ?œ$xbñ?'}zâޅ?†8œ"Cö?m¹sKu£?îz\x¸	?ª®§§?¤•ƒèö/?£ôòßõ¸B?–…¬©v|?"ãl¼åд?ë†ú†ªÇ?Á€ %(Ga?²\Øÿþ*ý?¼Ôç^¯Ÿ?±kRÉÑoÊ?ª‹$
Ó?ç Û2ÒKx?±6 çV?Åîÿv1#}?¯G…ÍuC?»'}]E?£ž9š§ø?ëÙ§Ýe\Œ?¤ïúÀ¤@)?¶'A?¢ öÀr>?¥A
¯?'qJï2?}AGN4FGL J1340.0-1501?íaA¯*ƒ@G›¥ãSøÀ;XB 6mÀ<®Ö0ù@!j¼<ܪ:?Ûeºnü7?àcÞÌ©'^?îȐB@™½ÆŸŒ"@qëô…M‡¿îôŽŠïˆ?ïñ4?ø"z¿êì>ý–Ä'?²Ë;A
€5¿Ñ΂#Ü(4¿èMnGÜ7¤AGNbcuNVSS J134005-150314?îÆÄC;i?¬U¼­3Ä?tò¢Œï€?~*DÉöë?¡¯m	{{?©A*ÝBH¡?ïª2Š…™K?‰¢hΊ7?_ØDûÆï?qßÍQßË?xTĸ4D?"&ÀÃ.w?îڂv¬š?Ô儅‰?yMk©Âj?w™§)þÂÅ?ž\MÐñ´3?	÷]k¬Q?îMç'?˜Aƒí…¶?nVâ7ø³?d­êFuÔD?­ª=ï›Î?˜X"Ò˸|?î£F$7Óè?¡7¼ó¥yƒ?ƒÐÐf,(V?…8ØyÁ"? ×i n?AD¦Ÿ§Ö?îÝ~Su¦~?¤þ6"Ôï?|§rb¯Šå?›h?ž?`?&Xü'Ú…?"'EQ?îl;	æ?œÈ‹œPÃ?~xç\UK?€rñé)¸U?¬
<¼ö?š±ˆ ?싖v¹?®-spY;?q:1L¦¾E?x¥	ï'ú ?º©<
-'?®33ø¦²AGN4FGL J1340.1+3857¿ëûîJ 
@R™çW"À;3
s†
À<°¦°ÙQ@@§;N
@>Ü~ñw§?ÌӒy>Û2?Áîj@æz?îuà÷üü@@躹¤Ò?ïÿȂeJˆ¿ä­v€d¿ë]Ä×5¿à °)¿é•ã+³ã¿ïßÓo~=AGNbcuNVSS J133849+385111?ïäüä)[?j"""u?L€ˆÛ ÷Ò?R.	DK°?câù{(Ú³?ddçÆXU‹?ïÁZ*jy?{žÝDLÕ?Rö£Œ–ä¤?^'úoÂ
Ÿ?z•Böþ¦?wۜTÔ'"?îØ·½­0a?—}ÌUû×t?l‰È<ƒŒ½?uʬjv~? «ç¤s¨?–×<}?ïɦÂwu?XD%dÿ¹?eÌùí¹l?K‰4Û¦Ù?pF"%¨0å?Q9:üXÀ0?ïÈcnda©?zd«íVtŸ?_ÊÌ£×?bí?àHO?sæÖ<zî'?tô[€/e?ï9;–6Á;?œ¼Tïƒ?hz}â;nu?z¾qQ_8?•É=v--á?™"TØcG½?î(hÝö&? ")ˀq?zÜ?es7?€_Ý}˜¨?ªê3«w>?ŸO[
|è?ïI¹é‡?|‰Òe¼=?'L<‡°d?p«æ‡
Ü4?‹rÕ4¥N.?tÀ	ގ¶AGN4FGL J1340.4+6926¿íR̸k8@GŠpCßÀ;µ?ÇÀ<DZ«ß{@dlƒ¶ÙF@v†a®pÁ?̎	Ãx:N?ÂþgN˜¿?òMº°k@À"CÆÿ-?ïÚKäÚá¿jÓaL²Fu¿ë:ñ£EêÆ¿ÙÛˆü¿ïÿÿÊPË?ï½%?T©¦AGNbcuTXS 1339+696?îYVÆ5Xý?Ä"õú?Ââñ¯ã¼?°z'QÕ??¢	"#Ò~N?¼¤§a$Õo?ïÝÀ¯ªt€?p¥8!F€?@Ü0ÇÞ´?O"©Tº?nCóVB½?lçf€»p?ïFê¨úN?Œdã$?3ù?v™éHyK?hd…Í?'d:âá?†£ÅHrUJ?ïû§OÝu?'¦ˆÝžº¨?ýK	³›ð?	†Ä†?;†-"ëÙî?$žn pÔ¶?î›U:‡™?»Y÷`Q×í?53³ö?¬ûíûh|?œúÃuÎà?°}±G}?߇©F?'Qèё	?Q[¹"ð?cœ˜"5·?‹säOá™×?=¿'Š­?!°K?•>Ҕ0$ë?~iÌ% ·?'uómš²?¡ê†w! k?"rF7?ïïÊYı9?NÒÿ/¦%?9¾}³T}X?0
ÁâÂז?Yû¬Æ¶tÿ?KÐøn°AGN4FGL J1340.5+4409¿Æ¤vAzÊ@Q"¦ YŸÀ;•/§xÀ<©u¹À€Ž@"!ä*7?ù¶È™aev?Åʨ…DÎ?¬°Ä¿žLB?åš>o§WÈ@ùŸM㍮¿èìðùÒ¿U¿ï"8Á½z?Ü5-vÇ¿ÏöÈlàÿ¿Ø:ÀðÒ¿£-oàô³,AGNbll3FGL J1340.6+4412RX J1340.4+4410?ïÈTc.?uéy^-W?8¢`Ñ=ûQ?$çÀ²yò°?zKÌژ5?u¿` {Én?ï¼áԊ ?/d{~B?Mäè¬
7L?X`£­fyŠ?}Òx•`w?°`U¹C¦?ïI]â3f_?"OS¬zÉ×?T×m¼¨[¹?@ÑÔlG?•†ÌÚ±n?"G!°1"*?ïXmf­*'?ppòxÞ±?Qfmó"¡ë?>«ÇÙè?"ÛìQ+ԋ?p@hœìËH?N¹ ž?}¹a:£"?E¯–ò¹Î?9Lš»{Ôç?ˆÃrîÐ{Û?}4'zŽØö?ïMbo'¶?—'ª0}ƒ?YÖ.8å1B?bàïªV…?"¶OAbŸ'?– Á¤[²?îª×v–V»?'MlccND?[Ÿ'uÏ?Yñ‰.
T?¤yãŸ5à™?',­ÒO‹?îÅzÀ]?[öÔH?cb«9ŠÖT?X55ʂç?®x÷dÿH?I']I¹AGN4FGL J1340.8-0409?àO5ó,@LA]€ä–îÀ:Tò÷ÙÀÑÀ<^=ç™@µ|I| º?þ®³Ý¾?ÂÓë9Ÿ]ÿ?˯D%ɾ%@
jOv@'g…d¿ïԖZIør?ïÿþBe«+¿Ùì ºŠªé¿áÒ°;œŽA¿å®úS¿ïúX¡+ß,AGNbll3FGL J1340.6-0408NVSS J134042-041006?ï'ôÁß?Š¸=ˆF—?iz։.Õe?j՘ò®t?…$ñµèÄ?ˆú@Vå?ï'ÍPf†?Šb©QúFù?qÑpBڟ?{¾A¯Mç?†cóß$,?ç8?ï¤[z¶;?T5¡ñ~?~¢<ԒV?€¢ZrC?–"å["£"?‡Îo³BíM?î;s.Üó?ÚYÍÇL?š"ä»1î?tv Cp…ã? éÖoy9Ç?vñĈBŸ±?ï8eÖ¸LÒ?•~JÿDÓ ?'¯ƒ‡|À?"ÅvôB?)íinfb?'æUÆ`{?µ\e(?£µ'Âü9X?…R-óxö?i1H¬ª? '‰,ˆù?š6! ÍZ?í÷3Âi
t?Ÿdˆš"*?'$Ç5"g?‹
2wßP+?§ú`H‰Œ?˜VÄUð/?ì*Ú¼éU?–˜ÏÄ°?¨MðKG )?Œµ;L:?²'7Ö,³A?‹Ä&²‡¬AGN4FGL J1341.1+7433?ä†??#€@EI¾ó(À;õÙ7>Z¯À=8XÍ@!m¡™?ý>½c£>?ξ¿ƒc!b?±í{˜ý'g?èÙ᝿C!@Wê°¢¦¿ð?ïÿùJYQ¿ß ªº©3À¿ÝmS?˜j¿é"Î^G^
?à…ª.<SmAGNbcuWN B1340.4+7450?ïäé'ïö?Š¹*¸Î-Ä?Dgù.¼æz?=ñ'ö¿?‡@FÕK?ŠuÃäab?ïÝÀ±Ð5ý?np¦ú¶Û?@Š<ïäá#?Kg¢°é?n¾ÚÍ<É?i¡öòT
?î²%9†X?˜¬&w
(?‡µn–žƒ?åª¡ü*
?û~$Ãå»?"m·¼ºóì?ï×*²
âI?ZÝ×g¬ Ö?T
DŠi=?;…Ñ´DŸÝ?nΫ½g7õ?YìžGû¡?ïLvѵ(?™¹r)¶?]ö>¼¥v•?XâèEåĖ?"'ÁñÂô‰?™_/œm?ïŒ
n)?‡èivÁFj?T`ÍX	—´?^uŸÈ<"=?ŠpŸþ¢,Ç?†	ðž×ÿ­?îKbOå?`çÎTø?‡U"Ò¢‰3?Œ5(ÛàHÒ?©Õä¬-[?™›l£.}H?ï"jh(³R?vø–J àO?e÷Y¤W?YJS'?‰gŸßVL?v¶9¸‰AGN4FGL J1341.2+3958?èח˜•k@RaÞ¨—cÀ:´4'D¤À<ÐÚx†ú@ ›Ó¾®{ÿ?þUÃKCË1?¿£«@`¿";$wj¬?Ö¢WBÜôb@üP#ÙÎé?ïúÖ*C i¿à*·ß)ñ–¿è?¯Èe_¿¹¸þæ$¿×ú3ÂûڿގH,¿{«AGNbll3FGL J1341.0+3955SDSS J134105.10+395945.4?ïÅa±Jæ-?q#ÅO%'?ODî$ÜU?Dö0b§ú?yk>ɶŽ?pUÜõö§?ïԝµ¡Ñ»?v³ïÌM@f?D"R'?Kút(øá[?s/`é@u7?u€ŒI¨TB?ïI2D\«?ƒ;œX¦¸N?b8àè~×;?[âHü‡´?"'›O[šÌ?'{!‡˜?đ®­?jNC
ªG?mÌìâ'?S"&'…û?†ÛÌ¢Ž?g&K0d}¬?ï?}̒?€ÞLÈûÈ?Ys=ðìˆÊ?NíTXÂ~?…·êVdU?~Ø7S¨=?ïzƒE=™?Àe¶=>O?X{3Û*YÚ?d):´xlt?ŽOӂ c?‹ßÂÑSø®?îg$±‡™^?•½æ±Î]?jÁÓv>‰?cùBt5[R?§ìèÌÔ0?•Jiœ:?în®o¥»?†+m(?‡}0®›?w;§3f?¡ÓOm²}?ƒVÑ{F!AGN4FGL J1341.6+5515¿‡ž·KíOŠ@N7°ËæÀ;«GhGÀ=Í 1cO@˟P<ÙO?ÿ0–‰B?Õ6]ŠÒ?ÄAꛔÆv?ðÖN™@°	j¿ïÿ3Qf$!?ïþ5$¤ú÷¿ÉŸF—> ¿ÝFéÞÖd¦¿ì.U'ÙŒ?¸Y:®Ò'AGNbll3FGL J1341.5+5517SBS 1339+554?ï}À—N*?ˆ'pB™hØ?s¼˜+ðE»?p¾$"Î?†ÞÃÒú¤§?Q"·M"Ñ?ïË éÞÅ7?sÞ+Ï{¥«?NO‰D™Ø?TyÄè"f?ve™öUn1?p'Á»¥ËÀ?vŸw?•_†£GÃ8?€EBé'dÈ?~§ôue6U?¢õ>я
Ö?"©¢ŒmN?ï•<÷›ò(?fx<ۈ;u?qEé•?U–qnžÃv?'-¾ï/sn?a Zß7É?îŒE Ñ¥?¨@>2»u)?‰aŸ½"Ÿ?ŒøÒYg? æ§€—R?¢I]S-©¥?ïM¬a®ï?"=цjÉÀ?c`5Ɲ ?u~nðv"¼?"Þm·U?'¸Cè],?í›âd"9?¡i0Ò"%?"ýXœ(‰?ƒL²Aýl¥?°@€z™?ŸhQ`
{?ï^qqÔ¦?'Âãl±ç?{xs{þÎ?mW&K{ü?™
ôºp?€šŠgÇïSAGN4FGL J1341.7-3907?èìr$hGÆ@6·Žâ†ruÀ;›¡Ÿ!˜×À<Á_s-F@!ë¹½ûN?øŸåÉä?ÖFlÊS?Ĝ:HPPÐ?ên±XÒÿí@AP5ÍlZ?ïâkªÛ
¿äòõÒ-_¿ïôo"͊?ï­œ®÷пë‡ùÞþ¨'?ß¾F!L€âAGNbcuPMN J1341-3906?ï"Òç)U ?Ÿ'Ñ}¡ñv?dÂàÖ=:¨?`É*æéo¤?™
G鋪?žõcÄËv‹?ï»ýê|
=?°×mšU?T¬BXŠ¿?aóN,ʹ?|Õú;¦m?z7k¤ab?íš)HÆå? ¹–.'™?yÀ¦2¸Ë?}ö}l¿'?±'«Ué? E÷ìAN'?ÝM£w?xÑyŸF3m?Upj‡̭?R¡<ž?†¦;^=£?wø⛽'?îÈ#ÂýÁ?£9J+JÆ?rJÈÏ´Ø?q#\¤¼OŒ?¡4j´·~È?¢a/~w[?ï8^lX)?¡Ôâmr?c¤PÞ;†?rƒ&?v¹Î?–¨_bĤ? WÂî(qv?ííÃgs?¢‹ç"ó?€Tûêý{u?*øxi?µÉ›w?¡H0ϹbÎ?î¸è'àÞk?•±'™Ï
?t€Ù_|oA?|÷¸§H?¡ábW¤[Þ?"–Œö}]AGN4FGL J1341.8-2053¿Ùæ™&­@D:[–(ËÑÀ9ÊàÆ~ÔòÀ<†Ñ?ù@ÿ¶YÃÀµ@t"« «?¼~)¦—ƒë?½[K?Äf!?ú4§Ý);c@®ã‡¤z¿ÝF—"Ûâ¿äñiϧr ¿èÂSAp²¿êªüóF¿éØêýºU|¿ðAGNfsrq3FGL J1341.9-2053PKS B1339-206?ïù󍚡›?6¼Åë¡?*ÊùŽ*¾5?gˆø³?Aߧï|?2Ý\½ŽQ?ïÞ!ŒD®?p%*]Sô›?A7^çá{v?JH'w}ér?m'¬n9?kã.~(ð?ï­89ϧ?u[I查?a 5w|ú?eFµ~[?€U$ŽÆ}?qKJ™êÁç?ïéLðH§å?CÍÞ2Ox?D+jŽ¾?'§Éh_0å?a¨+úÿî?AŠfŸ¯iE?ïòªõëÒ?u&'Ôï9?='"«ø/Ò?`úÎÐKŸ?SEr™†>•?iÕzà	Ú8?ïŠÕÑ$¤?jføæ#?S;aoш?_Aú­Wï?Šã‰-ß?Ž2X¯Óôˆ?ï^«G¨y?'Ý›í(g?os‹Ë¢@·?qe3À\¶?<%Žô"Õ?€¼V6Î?ïº$¥7Õ?h¹\,N±?`Ô{µšo?M¿Ææøߏ?zƒo|âÄ#?d¥jþ¯äAGN4FGL J1342.6+0944?äé']ÿÔ@Q4Z_Çæ´À:||ûÀ<€"ï5­a@¬ƒV6C@‹°'ݾ?Â77º+Šr?¶ÎùwМ?õL{ÃŽ@ª²W*´4?î°ßóE2¿Ó֑ýCD¿àéâoܿߥk*±¿ç2F8Éu)¿æ–øÕiSAGNfsrq3FGL J1342.7+0945NVSS J134240+094752?ïÙώÀo?]Á"]d?H¦_ÅùL?8˜óµ?plšR¿$?[ž¾?Âî?ïÌ3%WŽ˜?uÓNFäÝ?PXa
ê\?WêZ'	?uÐm'5"?qÕÎSÖ¸?ï¶VW
äò?cåee+ž)?UÍõ!BÛ?Aÿ(TüUÈ?a!îU?aóo+7t?ïe-r:@T?hÃÃ'¡H~?}Õå "îº?[Ç
M€?‡É°áÕ_¨?bšê‹Qgß?ïÃc¹Û$÷?lŠŒÝdÐ?T®LÒÁ+?E³z¼]?y)÷'ƸH?i÷=Ë$ô‡?ïn»¸¹€¦?¬jºZš°?`ËóιJ?hQ4ñ§_?
sœ:ü?Š=2¹±T0?ïƒY™Np&?ut¹|Mí?_"(uÂ]?MÈϏ™½?‹Fi1LF?sA2i҉'?ît¡·—¨Ë?'æÙ]åÐ?'× 	v%•?t5Øl,?Ÿ"©
sù?~Lÿ-ŽUÞAGN4FGL J1342.7+0505?ÖÂ-ê
Ë@P3 ٔ[lÀ:…̹–nÀ<z
Á$"@´¥§nïL@lFD‡ïM?¼èÁÊæÌ¿`àéè?rï‹y×m¡?ÿÓhõâŲ¿Â´†…ß¿ßíÞҞ¿çpLÎå«Á¿ãAãÀe»¿ëp8à?á¶?Á8AGNbll4C +05.57?ï/ª§€Yy?Œj×Ô·z?m®pFá$@?_·¢¾8cä?–TÝÿÆK?Š|ÃDϦ?ï›-dßu?ƒÞ·ÊNÉ?\øÓülþ«?`7‰"\X?…•Œ>ž=œ?'W‰Ý™­?îå.ù!Ñ?'; ÓºF?~E•Œ¿ ?|ã}Ýã4í?›ÈÙÚ¾'?ŒCj*Cµ?ïtà ¥b·?kXýµp?x¼)«èÙ?[µ¬å»?†iÃ8ç¨?câ:‹›?íÿ	A=?¤¯
i¸?'@Ú–È?uEUzÕç?«9^*»?£hEDÔ-?îåüʈØ?¢ò¯JàíÏ?p«œ9&?•"º'QÕ?Ÿ9úûóѪ?¡¦ë]MçS?íÅ̎6V?"¸]•a›?‰èKš|%?…)µÇQל?­)/ÈF_ž?™ÚÏY¸ç?îYŠæ«ù¡?‹J;–Î?'ÑRÏx?|ïPñ0?¡eE¨K{8?ƒ{ 3.‡#AGN4FGL J1343.6+5755¿ïò{½w@LïQ½aõ¾À;CP8&·ûÀ<ÃÕ×7‰Ú@½ÃIâ¢@ÊOv`?Æï8&&Z¿"-"®jƒy?½*¸TÌ`@ëÓSú~?ïÞ>y¸R¿ë³â…›µÔ¿ä™V³jû÷¿é©YàÆÿ®¿â7EçjÞ¿ïú°€²AGNfsrq3FGL J1343.6+57536C B134209.5+581020?ïèq¨†=ê?dXåÙ¿øŸ?9ÀÔÿ ?2*¨zQµ?dVV'¢ž??c"Ûå€
D?ï··+оI?‰Cp'"?TFy¦%n?bi@θÈ|?ËÁUfŒ?‡gl(zÑ
?îÒO¥YÁ?–J®ªö^?`-*í;?nÂ,.ý?¡ÜɱCÂ=?•ê%¤ß…Ó?ïâò'œž~?Lí_bo¢^?I4b.¼gj?4þ?ø×ï?fÀ¿ÈcG?H؁÷yà?ﶘÂÑm¾?‰
f¤–?H±Aþõ=2?F"c(·k?€Î»;ä2s?ˆ)*×Ö&y?ïAä²$]‹?–]®$ù±?aÁl`?I±?më¿ o?•‹<)ir?"fè{ÛÁÓ?í庭C"G?ŸFfC?dÇ¢Q?g³_äp?°1bWë?Ÿ6£4Šçž?5^Š?p{N£NÁ?e¾uA°¯w?Xÿ3êü­L?"(JýmÁ?lˆ¦L›g7AGN4FGL J1344.0+6605?Ž©Em¤F'@I™" äÀ:›wTË3pÀ<«"¶
+@–6ükuð@äìé¢Æi?¿8Ȑ‰¦?°£€ùÊ?íºÞEÆ@|™ÒÏp@¿á¹€¦ƒ¿â³Eqú_¿ççb\«¿æ¢ ©XS~¿â¦t©H›¿ãŸsbÎ+rAGNfsrqGC 1342+663?ïêv΂H?XãFxï±Ò?>¦gÙ1p?0øõW՘?b¼P?V«0É58}?ïÙa_E?n]¼_]?Bò!õ`È?K	{ªÌl?pñ.ž€?iü?	b?ï¶UT½?msŒØS³B?U.il¤œÄ?Sp!‹KP?‰ß˜ÓŠO?jÌAd¶ÒQ?ïÓ:Ë5¦‰?RP'¯Á¬d?Z¼üsÑ,‡?;×HBð
‹?of¶	!?Q@­Eþ$?ïÈTŸ}ø?o£"È;D?Q]ù¬;D?BYŠ¡y¾H?w~2+"?mÌì(DE?ï<°#bŸ?þ—Úƒ—ð?Uٛ­¿7?_¨Žo?u s±O?ŒŸj±Šã?ïr:+í;$?AS´irð?`Ú_¡ï3?Qå*f°ä?:Ý$º?}DŒ4Hâh?ïm|Ÿ…8[?t\zƒ|Ü?u›»î:S6?`¤ÍWÒ½?‰Òú3Ck"?r?å˜AGN4FGL J1344.1-7700¿ÕgiÖÀ,è鳍aÀ:j{Ö:3ØÀ<_ÐJ/Ï@dá59°@ðÏü,5é?ÇߋÁ>Ï?Æ˦‡ÙL?ùÂ=ý'·?õÂ/)ä*¿ïïwÀOç?ïþõU9¿æRÝ^ˆ¿í©·ôÎs–¿k*ýžj¨"¿èk¦âWxAGNbcuPMN J1343-7658?îA)s÷8?©}A ì±?'I./-ä?•¤£ƒ•[?§[CC÷?¦}º–Äq?ï/éÆÇhú?RE_˜?)ú'"B?Œ7Ⓤ@H?'8…hÆN??"ÕEê$?í#Nõ¦?¡P»ù"½°?—û­•6ùà?"'QÑσ?°å
!À9Ù?™ÀÑ5V?íh{®; ?'ÄþÆF?Õr0ö¢F?h<r¬?±tIS6?¬¹˜"Ý6?줄H''?³Ün<‰ù2?"µDØø?–ŸÍh½©?µîœ¼t÷	?±ƒ  'äÍ?íRÿÞ5ï•?·çö«LÝD?ž)% –i?®&•¢p?«»oŒ'»}?°`͟Þí?êìj"éù¦?¨ã¿ƒhHÌ?§ýQ©.Ѿ? Râõ×?¼ž‰óv?£-Éñ3&?èÕ¬ :%H?«'$É×?¤Ö¢UÙ:?›uÁjsú?Çs¤ê}X?¨É!þt¾AGN4FGL J1344.2-1723?ïýÞ¨v¬@EÕ¡"úÖËÀ8ðÍ¬üÀ;Õàl¼Á½@.÷"ûR@ÙªæÈ÷U?ª´vØz?¿-¯e³¹@ORáNd@ãؖÚw…?Û´;ÿµ'¿Ùs8œS³0¿ã'Í¥&Á¿áš¤'D`'¿æÄì=ÖOX¿ðAGNfsrq3FGL J1344.2-1724PMN J1344-1723?ïóÁ7@P?N)Ô¼T=?H¾‹Šü¿?C¬G3iœ?HàdfBØÈ??WDr?ïÚB3VC¯?lAÈÇ?Dâ&bK?N©þ¤áw?pB"°ÁË\?h;#êX_{?ï\PÜ͇?[ñ¼r?€27'q¸–?…d­m!?ˆ¹'TÓKT?†øÊç?ïð֘c'?Aų̂ïòV?8¿è†×°|?#´Oš¬›?X"Õb¥O?>]™{9"2?ïë
BïÏí?\¦ãòÜ ?S`±å ›Î?T<ùv?V"È'·i1?Mý¥	æ'g?ïHZjbR?Φȁ?X檒9üÅ?nz®B+GN?Œ'±Ïø?‹&Q
z%?ï!.
ÕF?"ìf¶'y?'ª·à?‰:©"ŸO?'Øi¢«È
?u<¢›?ïÛd¼\ ?^ªûçx'æ?LöáA?<¯§
Xß?m]'͍•?[uí^'‰AGN4FGL J1344.4-3656?í-ž/Êå@8¼%á;ÛÀ:6,PÀâ´À<G‹³ýÉ@Y/'éA@£Cœ7Ì?¸Ñæg'¬l¿tª÷ºâ?ã_v¼Ï)@:î¿»Â8¿ÚËÅ:Ý ­¿äpŸ¥LU¿ä´àFý¿å=µ¢ä›ö¿âŸÐJ/Îû¿Ô‰þ¼3!•AGNbcu3FGL J1344.5-3655PKS 1341-366?ﶲÿZW?pj8Cú?]	Ñ¢Ž?I'}ÍqÌ?}frr/¿®?n$ÊCÁZ?ï¼â0â ?wL –UÈÜ?Râ½ Ô ?V (ÒШ•?|Ö8mô?t]ú¹D‡?ïBSyF4d?'RQÜ°B?s'Wv!?r‡‰‰" ?'óp<¸sù?|X°
îGP?ï]-ïŸ?jCµÁSV?qÐÉsuü?RÁŸej?ÐÛ+2©c?gS–²ãÝU?ïTíúç3Î?'98VßÞ?tzM•>?cÛvwòP"?Cºå¥¨õ?­›x#Ï©?ï8†ŒK¨J?'e2ØÇU?i¢Âz÷âŒ?p;‡'™&?•ºÖ/k
b?X"I?î‹#HžC;?«sž£½·?€ls]Õ$3?xOU'…WK?£2®¢ò8?Œ1áþ>˜?î=¸GY±?ˆ‰UÁ·÷§?Š­zž˜?t*?Ö÷?§ˆy¾¥ï?†qm'à*AGN4FGL J1345.5+4453?åQ ±Ü1@QM#c²WÀ7&Š
4›éÀ;q%SvŸš@|Bµ²)@^á77¥?‹›ó]|ªB?³øf>ßu@&y•în@ »ˆb¾¿À
lÐó.¿à Êƒ+¿ä²+@ "¿äk¾§›¿èÚ^Poˆ¿ìܞÁ̓—AGNfsrq3FGL J1345.6+4453B3 1343+451?ï€9óä
N?‡•‡Œš»?gy"l<ií?a*åÕ/
‰?Š ï'3?…÷÷^K?ïlWœý"Ù?–ø{‡º?pGʌ†+Ã?«7SæËh?ŒÆ3j5‰í?'˜:èÁòj?ï›ÝtBz¬?‹%…Ô'?yó¤y‡Ûu?ƒÎd,ruN?x¡R¬êi?þHìí!?ïòY×6Þ?N»¹/³5?I;i´"Í?BT:
]?M]9©?>áÑcrJ?ï^⺆	€?'éQÕÅÙ?c–¡4 %?]Õ&$Î?'°ÔéÜM?'kð"™0^?îŽtj1*?°Œ¦f艚?'03½‡`?Ÿ±Ùi ?¢Œ±a&Á?©¡–b3z!?ï‹;Üu?‹Q£ÓÝ¡×?xÏr]±\<?ƒ¬£4> K?€É€W¢U	?ƒAAåvg?ïà¹<»áÝ?cI¦!Ã?Zg6(?U¡È[ˆÅÁ?b=£¯5?ZY=ÚRvAGN4FGL J1345.6-3356?ÀºXO'&@;—BöÖÀ9ýžóu®À<PS@ôÄ@¾wÎm¶½@W]K4²?µž—°5gk?"?\6a»Ý?Ѷ»"i@+(wÃ[?ï÷À@win¿ääž_Ñ÷¯¿àýXsHͿ㣮¡£S¿Õú7¿	Ò¿áž$˜¼AGNbll3FGL J1345.9-3357NVSS J134543-335643?ïÚêéy¬?"q±"Îc?B92¾P­¡?`8㛠O|?pC˜ÌŽ:J?'Š‹ò'?ïçÐ$V\¿?r?CN–¶?5¬‡9P?CæF€-?ez[Ù¢³?pú 4ˆ[Ð?ï #v*?zœ>µS{¬?YÛöϸa?g(U€wû?"»ÖwžÜŸ?xc}Ø?ïî@ø=,?Aa=p¦?'V$=Á?
a_kâ>?`IŸðœ-?A[ύû|?ïÄ"I+0?•Û›Ýñ¬8?Q"î²xTO?f"ìMúi}?y‰ŸÚÌ?"FÎû¹ù?ï´\nsƒ¹?ƒ²ÝyΑ?H'|‹ÁÒ?Wx Pï
?_¼¦«z>?ÐŠ2ÿŸÉ?ïDÀùÒh?ˆ—œz…¾W?a;|y
?ecC—gŽÒ?•@qQc2?ˆîµ˜o?ïΫU?bîzO?>ªq&<?)ßÂçt§Ã?wn¸¡?aÃÈ»FòÁAGN4FGL J1345.8+0706?ßS–Æ疹@P‹6¤û©À9lì®êc·À<7T+Ñ?"@‰gWË@P†å?¯6lx¤,?ªíŽ
t]?÷@ô@g)™¬c÷¿ÐB~ª¿ãWZYé¿åÎU-XþŸ¿çí`Á
ø¿è¯>;¤ò¿áìÈ×'šAGNfsrq3FGL J1345.8+0704TXS 1343+073?ïöŽ!ôÏÿ?Mù<#ƒ–}?0ïԁ†a
?/ú$×wa?MOŒçgBÌ?G²]ô#q?ïáŕ 
<?nt¡Ð½LÈ?;Ž;J/À?F¿`"Vƞ?jȪÖé=i?jË&-‹w?ﵿZÖ]?vöf¶±Å?Y…#"®??_•Øàf?~ÞO'ò¶?uú—iøD?ïú×÷Î-?+¹Ú(|ö?+&_)«Þ¿?
Y\C¤?@ǵÔúm?'s:>î€R?ï씌OÀC?`½±÷Þ?:¬¡S¨?5pV¼Ó
?`ñL
¯?\×5Bj ?Éñ¦ ?"^dz@–?KŽçZ'³?Wòt¼Ám?…¢^þ×Ц?ƒ(ÞWÐ?ïs'´È?"KºG÷×?aÎØ˟¯j?\"×˪ú?ŽÅiw²Ð?ƒ"üڈ®"?ïïâÇÇ°?LZ1Pnu?C8WÒ§"?4L›'"W?Vžp
o,p?G%etãԔAGN4FGL J1346.3-6026¿ÊëÏÒ1?ûL'à°«À8q¡ueÀ:¡6¢S|@''•>@-@˜ÿ%­B?°üñ>~–?»B	å²@
ßËâ˜?þªFJ?ïÿÿ" 5•¿Û[gð$–¿ä¶0íÖ¿äù'c€¿èQ
I/û¿éÊßâ©-AGNrdg3FGL J1346.6-6027Cen B?°ñÞ'ˆÈ ?§¹ì¬X?'SÎþÊ?"›3&çÙ?íMAœ''&?«d%å?Å%éÀðÃ?Á,ÚEÂ?Æ|Û.´?¶µí³p\?å6—NÄ;â?Š9tÍ?Í[
WE"?²šîNî¦?»Þ:w9S?¥½,}®Î×?å-vC
5?´Ša~ôG}?Ŧ9Îõ`?¡v¢"àá?¼Üý©Zú?"(¥æ"?æúÒ ãe?¨^@'Ý?ªYÍX'PE?¤ž_apz•?•Fc;¹"Œ?"t
½m?í°0‹_ç?©ƒ¨æ?±¢Ët¯?±ëÜN`ed?ĸd—яÍ?À+£Ð\×Ð?蝍kQÌj?ÂŒ0ûK?ÆоCB?«f­Æò?¸ÕÚqü?¥ç*GŽ~?ç`P'yl~?±VwA©8`?°¬~•r ?"èÒÎßñ?°‡Çµ
ä?£Gç¢Ëxb?é>N;;.C?ªßÁ*aOTHER4FGL J1347.1-2959¿ï̏»z@?[4ø/Q&À9ûŸÓo~=À<BÙÊQm@æÀ3â/µ?ý"ZÖk®?ºbg÷¶?»à€&(@t G2Ä?þØépq'?散ª?Y?Üg¬Óª7¿ÜxÏ>ìúÀ¿ØÍËz¿åºçÇúÖ¿×`óà·æ6AGNbll3FGL J1346.9-2958NVSS J134706-295840?ï´¾uh"E?oÛßæ5MÈ?W'/
ª¶÷?EkÈfàþ¹?À9ªot?mÕôÓKøï?Úæ…? 4TÊ¡h4?'¤Ö*ž®?"¾=©3¤?œ
^ÌÀ»?ìÆcèaó?ïZ8•È©¨?¯´=ªÊŠ?nU€L¯ó±?m;•íéƒ6?î=8Y] ?zµÏ&¶ü?ëW…Q>?¶>ž~ä??­ª‡pªÀ'?†7ô«;—+?¶r€GÍ?†³Íud?ïmÕ`ø›æ?|'8ÿcÖ?l(‰Ê6J
?Zœ­Ø ?€…\±íß?ytÁÕAJV?ì•"»…–?±Ã¶f*—³?£Ï¹à7Âø?¦‹çªS6?±oúãØÏ?¥lß¾vZÁ?îÉl^^@c?ŽC¶¹?{pTK8?y>nÔÏc?Ÿö_-½?ˆ¥¯*AB?æ'¬Bò!?¢äºŠmV?½¿úù¨Dz?š²_·kSÆ?È­»Ò A?ײýðfAGN4FGL J1347.4+7309¿Ùˆä•–TÁ@E¯BöÖÀ:øˆҜÀ<ʔøJ)@‰ðP4¡@)}Ý{pº?Å·?ªô²S.?âÍ,n@/†—3bÙ?ï)Œ‹"Y¿å|'€Æcý¿ëϒ_µ¿á¥Ù]ÔÇm¿ïÿü¿ÙŸC?Þ{©Y*=ÁAGNbcuNVSS J134734+731812?ïósT,õN?[̝tfü†?PŽ©ã«?Yz=8½²8?A[‰Ç?l?8í£‹"Ç?蠟%«Â?£¶JžA›—?Z5ó"€$?gRãó÷u?ƒx]¨µh?£'p}
©?ïzëyhÕ4?…Öæ²û5-?iåV
Ê?r%b­L¾o?ŠËޓ³K}?ƒ]5)Ë]?ïè²lµq"?G¡Áír?UŠ[kJ=?>\$mØ
@?YË\èÁÓ?<"'™ÁVÃ?ïçû¶ty?jªk/"?bCµ—fJ?i_)áóÌ?Gëo!&Ù?Eµó–Ȑ?ïd"»?¦·îFÙ©
?nšoz3?'+uÒ§›¨?˜à.zýý:?¤ÀᢕîI?îøXëèa?ýP€Ô"Z?y¸ùœ;È?~ì¨e1ƒ–?š®ôa˨ß?Ž!~Á+Lî?燎ÙÈøq?p..-9E?u ÌòïÀ?e¸6²U'ƒ?vžÆ—1?b¤ømEšíAGN4FGL J1347.6-3751?äôdjÛ£@7¯ŽŸj"óÀ:‡©­
À<ô¬å§@æ#·ë_@[r>á½?º™+"î?É)I¥e·@
£ @¿ä@™!ç±T¡¿€¿^Ð	A?Þë®9cÎÜ¿äßâSFÏ¿äÓsëUN¿êqZ€a¿ïÿl&™Ç½AGNfsrq3FGL J1347.6-3754PMN J1347-3750?k黤?'*¯Éä=?€À¾ç¨æ?x=Þ·¢Åp?{¯ÌN^E"?q2Ë]Ñ·V?ïϕѰXÅ?w>ê€wö?T¨ñ5?_ÉX*»ÎÎ?s--®×û?q%Eiؕ?îûœrß=	?'0sA>"b?‹¡øƒu?‹K0ט–?'»u›êU?‡(È
Yáœ?ïyÞ°Ïì?e"qÚtû?užÀ‰ðF¶?TyhGLOÑ?†¸ó•Ó*N?_ª\ݖ«?îèÿÓ6?•…9ák?•;.ü®?óJó•Ï»?‹IÜiŽ>;?€2¥ÏF÷y?ïnÌI†?+Å:83?gα³_Ì?rŽo]?ŽYzH/>"?Š´GPéªé?íàEÉý~_? ü#7δ•?¡·Óåq"©?™z":? CÏwFêg?'n"ñU"?îºæ±OC?BbÄáÀ?‰§ÆuˆÓ?oìñœâ?›Ï\¼D?{ŒÊç¹ôîAGN4FGL J1348.9+0756¿½GÊ)@Pì¿±[WÀ;'/Lô¥YÀ<ŸÀ_@˜@ 6Í.Çhµ@cpÍÈuO?Äái§c†¸?{ó¦‰?¸Å›€#¦Î@°Î‰»U+?ï!
÷9ˆ¿äi;,ü¸M¿Ü4…ãÚ/Œ¿êq¦ é4¿¼am¿\]	¿Á§Â盰AGNbll1RXS J134853.8+075704?ï³]üpºŽ?v‡Ãe$?HæZý`$×??°qõ'Õ?š1ý-´?uº{µ"»ú?ï"hŸ%0?Œvú<¯y?`S#kY?lCÏVú–"?†á¦œ¹?‡8r$o&þ?ïA¬±é?'i?ƒá?cۓE‹à&?e´Ì¦8oÒ?•N÷qׁÞ?Tä­ñï·?ïš9jb}?kçÇ[r?MMýD˜]?;.Á
'S?‡œÅžbe?k©µ¼×ª?ïiŸÎ3vœ?‡PƒP,X?Vx·'ü?I_T¥¦õ?'j© ~¹?†®?¢'œ?ïÈBŠ¥F?§jR¾š®7?e^÷ì'
T?tžj_H?œû«Ę?¦{ô	¥?î'\ð§?'"8+•…
?hk·ÏˆÀŽ?Y×Xt;ãD?¦S"3òD?'5¬ì$?î€èS´_?Ž]2°ãT|?f¯†Ÿ"»Þ?^¨êÆc i?¦†'gX;Ç?Žš¡X41{AGN4FGL J1349.5-7153?íUžìPÀ#¾è»¶À:^qS)rÀÀ;æ"4­†¶@:û³•V@Çc»';?»œ
7;€Š¿³ivRˆŽ?û
6 ¥ý?é8.¿å˚gõ²Ÿ¿áu³Á
&¿ìã4–~\¿×çâT1¿á½'á>sÙ¿ÖFÁ#>AGNbcu3FGL J1348.5-71502MASS J13490974-7152510?è%g€ö=<?ÈO®5`*?ˆ=ʉþ%r?‰²1OŠ*1?Íæ…RTz?ÇéíõÖ?èmwZ摫?Ã@!\q?ˆðãë<ó}?Œ‡$?Ì»UCöœ?™ éÀ´¢?èìÖú<
Œ?°ÒÜÎ{?°>ë…ò?‰™YðÆ­ø?Ê6œ:DÎ?¯Ìó5Ø¡?êr/Œ#~?¢N:úãó?š·ÕÙ`»?…¶:=¦?Â{`H•.? Æ²è†M?âNF»êì?ɏŒš­•Ð? s·ñi&o?›÷êÏð'?ÙTûŠOy»?É:â@ÉÁ!?àáh˜ßy?Ï(ˆ)¯¦Ì?ð¥Ô&Ð?¦XÞs«Wä?Ü^æÞNˆ?ÍóAmUs?äZv¡¿O?·_™jÀ5?›Ã u£<¨?'Э@»= ?ՏŸ
ØÝ8?¶Æ[>1#?↜Ž~Ú?¶ò<?mÌ?²Ü`Bs?£¦ØÂՁ?Ö;®ä¦Õ?µ–©ҏËAGN4FGL J1349.5-1131¿Ñóxˆ'u@HnR'ƒÓ_À9Ñ×ΈÀ<Ñqw;¡@gŽiâF@køüÖÔ?±`'?º×ù%Æ83@1ù⯍!@¿¨ƒÂAÙ¿Ùò½'È¿âYLV¿æ¡*òòÑC¿èò™°?ÎL¿éÓÔޔ‡¿ðAGNfsrq3FGL J1349.6-1133PKS 1346-112?ïô:µ´)?U1«®?68U)¯†?,+Æ¿`À?Qü€¾\>Á?RúTšaÃ?ïÞK>ºh?lñ8Ͷ¨?@šzXéÆ?Ng×ÕqB_?mŽ"ŒVÃç?iKyK«…?ïž^ïhqó?~Cú$ü")?c!>Íïµ?i¬ïÖ÷Ñé?ƒŸôc'	_?{zYsGû?ïùÒé5R?0'œ1	qs?&a¼4°€ ?gÕÕق?CìO?-ÐùÌ:F?ïèåA¢&?ZtÍÊz?CŒ¡3wîÒ?4ñ>«^x·?b7ÒHDŽç?XFÕj0p?ï‹vH[¹d?"ÉÆ¿í?QÆ
àÒ4?`ggê[?Šé¬+—ˆr?ÙWµù•?ï_ŠÞ&!¹?"'*}?kΖg?m¥×A§3›?"Ñw›0â?'‹ZSk"?ïï3ƒSö¼?PŒ¦Lˁ¾??²¢al?0Bâ}	']?YÒôÛ¾êý?LÌö—
›AGN4FGL J1350.8+3033?â}íRö"i@S#'©"áÀ9¡%t9ŽÀ<xáR•Ï@F•[œ]ï@ÚöƛZd?°%ºç?·'.~SÔ$@f¡aä÷f@"·wP?ÒXÖ%;"ì¿âRñ©ûçm¿ç8⟜é¿äc²¢)5.¿é'ï~R–P¿ïÿÅbu@AGNfsrq3FGL J1350.8+3035B2 1348+30B?ï…
eÄ*?·ß7k»µ¯?G!¶¨'?l]©†P+†?J‹7­Ë"?·Ê(¨ä¼ã?ïÝïîÔ£J?mnâC©
…?? e¾Í«i?G"YHôÆH?n,CEIí?iëåØͼ?ï¸55i2?q†tòÇèt?WXYå!øæ?C<òiü?~YëRü¬?qE¬ܦÆ?ïø÷ @Ÿ?/Þë€Vù?:éG]ß?#
úƒ°y?=ZéäG3?%>ò<#uÆ?éöºm?³XÌ£³Ù?M‰iÇ'??›pE^R?…FÜí³?³]üQ"©?ï›RK§HY?†áM7?Sƒ¾ëR"à?e]2CGË?†ºõ+]_?…}}{£1?ïl$tJø?ƒ¸29.'?eÆÜ÷Ö?bM(X¾"?¹±óõ´?'N<I—ƒ¬?ïëô±Üö*?Ph‡4–!?SÏDŠï=Ø?C6PEQ¾?TGX
›³?E2'²ÚAGN4FGL J1351.0+0029?ê]ê–â/@Má;:h±šÀ:d­
ê¤NÀ<jm÷È@¡lÅûø4@âmæÎ?ùY}tË?¹•þÀ¡§?õ%b?8È@vÙÑ4¿Ÿf…Åý$Ù¿ä	•ao1¿æšÔ,<ží¿à¨1ý©
«¿ïþpHgwÞ¿êrÀü§†AGNfsrq3FGL J1351.1+0030PKS 1348+007?ïò]h÷÷Y?J¡7?Õ?8Ö@a&?§?(õ]RÅ{ä?U×Üc?G´¾Éz[?ïÞ%ÒCü|?oIùÃWÝ|?B12Nã"?K¿ô"PõÂ?mMá†<?jªP¿î¿|?ï½oë±z?jFMK -?YîâÌ=…Ç?I
åÛޕ?zÌQ_•¨#?gkühsïT?ïî@Pص?@ÿ΂Îý?D›•/š'?*×KYŽ$B?Ywրx‹?;Ɣ «y?ïæä.×ó‹?[AjHB?E›$‰D€'?8=£m³Òð?cµ/ƒa-?WqžöÌ4×?ï– Ñf?…1+â€?S§p{Îç‰?_D½ê•?ˆ©Ë›w?ƒi§È3EŠ?Ê]±·?|¢l
Ȇ?càb?3^?`¾"¶Ëp?‰$4ɨƒ?xÿ@Xø?ïÍþF}¤?`õ¹²6?[x2";‹»?L§­@bÌ?r"ÐÀ4®?[ØãΟAGN4FGL J1351.3+1115¿Ïs†žj@Q1›€#¦ÎÀ9t™kvp À<
cu^P@…oòbü?ý+þ‹‹º?±@¥\ˆ?°¿ð©Jè@¯\äÝdË@á´¼µ¨n?í°çɨU?¹ðQJöH¿Ü"÷ž\¡ì¿ß"S¼ëƒF¿Ôk•D C¿äM~8C"AGNbll3FGL J1351.4+1115RX J1351.3+1115?ïˉ˜ð|T?wî»Y9܊?J'§`:Ær?GÈwVvè?vèއ©'è?uq‡Â¯¥
?ïÍú×ç¼?u…"_:?NX¥Àƚf?V<ú–cv?u7ãÜ\܀?qóÞ:[v?ï{Qî<ç›?‡Fkø‹<k?Y†›¡ñÖÁ?_æ#´‡Õü?ú±WR~?‡äÝ´+?îñ&ï
?uÞUòa-?€/,Ï%Š?aðÓá—ËÀ?™Ã§pXø?r†À䁊?ïG'Ž[ÅE?£z}Ÿ"Ò?föKkü6ú?p¨[÷ &¦?"<DØ4"?¡¹!ã[?ïmY»™Yê?ks™Ë[?c_i BÔ0?kÆŽë·¿?Ñ¶Æš‰?¿ÌbS8?ï_åeAp?'2­EUÇ?`pw˜yŠ?`h¶ÑyŒ?›ôk	Sà?äÈÔá?ís†¥K(?'uI&fP?'pYÎ5T?~r²÷V?¯¼Ýzö¿…?ë-©êSAGN4FGL J1351.4-1529¿ïÿë€}@F|SŸºEÀ:}«fJ·´À<`š¡×U½@­ïõEçÁ@ÃÙß?Á»»?™½)Íó?Û¦£Æ™,@""ì¿ÞB#ßX@¿Èš×‡:òD¿ä1YtœU¿Ù"öd ¾|¿ã\YýL¿Üß齃AGNbll2MASX J13511746-1530155?ïÇíO¬Ä!?r¨Ö‡tƒ?MÆm1uAR?B'hÞ|³ž?xPŠŒrL?rMèÇ?ï܁¶#)?pÉ¥Ï'³?AÛ8âé=?K]–ó?o{ÍÀb'?khš~Š	Z?ïX¡Šîu?Œ fӣʃ?T Mæ…`?Ww('c_?"º†ïµêd?ŒJeÔÆy?Ñ(?`û"_qîC?[ӝ[¦?9{‹µ«€?ˆE\yªE?`É«)í™?'­'|?‡tUÀée?\Ÿ‹€d.ø?YýÙ_,`[?ŠBééÑ?†Qå™Û‰?xCð?ˆr––?Rë,þ͐?[öèÆÿ¶‹?Š'ž†FV?†ðf×eÝ?î¨ê_ãH?œa]ZQš?XÿúU¬éÝ?T¢ïps*#?¤©Z1Ý¿?›ò 6õ=?îÅ'"9?f¾æ?rŠÌ{ȓ?W¬žÎžže?¡\Bã3Ô^?
Ùÿ³AGN4FGL J1351.7-2912¿Úڒß&|Ó@?օ3±tÀ:J4ÿ¼
bÀ<.43
s†@³Ç­ËÖ@=•!dԖ?Äab*Âv?Ð0š<+ÕF@	¾È'L@K8P©f?å}d¸|߿߀-·É/‰¿å+¦—㷿噹Å¿ïÿúVrÓ\?ïÿÄ`"AGNbcu3FGL J1351.7-2913PKS 1348-289?ïª~Ë%òr?~~Uf?€A6uĽ‰?{Crá–?d|ZÎÀˆj?]ÿ­êEn?ïiÍñåàð?'ÎI®Ý"?w^bñò¸"?€KÁ…O?‰ÝR}cç?†:k"às?îSy—ϼ?˜îíÚØa?–SXB?è™zóÂ?Ÿz|1A?'µº'˜O?ïhr-!©Ñ?w&U¦?vD»Uü?\àsyE¥t?ŠÁ¼R2?uPX×þm?ï_–¬26?EùS?3'BÍËt?Žš4ý–Kå?nÍA¨s&•?d6êцL?î¼:ù"*?¦
U¯8I?"p{næ ?'êTOÁ
?ž@~—¬üÅ?Ÿž ÷MR9?í?±ygÔ?¢«˜mÌ@ž?¢Ý;}_/?˜¬;.j¦±?«.ÉXXn?š9ÒÛ¦ý?íéÉîÝ)?ž8ÍZfS?œFÞRN
?ˆVМ?°ú.¬Q1?›[ÍAGN4FGL J1351.7+5542?éÐärø@M´¥œ[dÀ;•Ùs¤<‹À=<ÖJ$@ŽššuŒŸ?úŒõ–ðqî?ÒÅ%îÇÉ?ã‡/iz@".C	j@´Äî1!¿Ïì\	@E•¿ïZu%F?ì_Î1PÚä¿×álˆ€Ã¿æSÿ¨Â,¿ïÿøþÙå9AGNbll87GB 135011.8+555656?ïÐ&pØc?vÜ~#ÿ?dŒ"VxG?e"W·lÁ?kM}gTm?lb¯}Ö¢h?ï{éÔU¾_?'9–´êß?piõàiÿ?yD
¦Jx?ˆ÷ÕßÑÿj?‰¥§vÉW?í_ü…TÆ´?¤9ä{ŠÓ?˜ÔÜ 0_å?"Ý-È.:M?­•É[wKÆ? |ôßoό?ïoáZ+"K?s—Ç3'?z`ìՄïý?gàÀ°E?†×3	6?iKçv$¬(?ï{˜µ¡•š?ZnEñâ?}æaUÕÔn?"'JV¨'?'&¡ß¡+W?'(úŒ[j?îcÁއ4g?°ƒúa_µU?†ÌŽÊ™Òá?•Á'ˆ½¤?¤¾gyùÑ?«<ŸþR?ëÒŒvgÞ?¬H¥ßmÑN?ž‡þZä?–Ö3>KJ?¹í9ºòë×?©q_w|?º54Y?'·"G«›?ˆòsþ¿?€ÛÀœD7?ŸóÎÀÙ(Å?Š ¯‹¾ý'AGN4FGL J1351.9+2847?íKˆd=a@S"T6¸ù±À;' ŒÒáºÀ<î%ÎÆ¢@Š·ÖpŠ?üýŸ‡Ü?ÕËÛø8á?Ìmñ	Â÷a?ø¢³ôŽ²¶?ÿ¿iÒ~¿ï¤«{Cm=?ïëu™àv¿àkTñ¿Ðü¸''ì׿åévP¿5¿ïÿ'R}{AGNbllFIRST J135154.4+285007?ïÚò¢P?a¼.Ìː?PUJyŒ?AÅ&ԗÔÃ?mΆ†zž?^"Þàù:?ïÈ8ᇴ?y‡¥t'[?Q)·úyÏ?Y™ò4†^š?wœê^O¿?ur™:§-o?ïE²-S4?…±-ËD€?ot͐KÒ
?ld¤ö:J?"[ ªGü>?ƒ9´D~SÕ?ïJÎ~í_®?qñPt='Ó?X€M+ý–?e;ùÍ®@'?‹óàÔ?j(–™ð¼?ï¶ÛuËÎ?z3ŠrŒ?^3õÁ,%?TóÐdat~?}p•vÁà?v΃-3üD?ïAÿ6"ô?—[ƒ¼ì·?höLáR?y¡ÕÏq?"±,i\¾\?"uŽ63ú¡?î¿fŸò#I?»g•R?wAƒ?q³…?"âO?¡(5x8Ê?Ž~ì'·ë?î‡å¨6À?‹6–ü¢•?‰îSëE¦?}s)ð¢ÀŽ?¡
@Â'?…¥<¤›â;AGN4FGL J1352.7-2742?ӄsá½äk@@œ°À&ÌÀ9ïHk©œFÀ;鼌ã©@‹¥ÝIǟ@M_Âví?ÁlÙ݁zê?ÅPžéd³@é¾àzÿ{@]¤í_¿X¿Õ8~âHN¿èJ€Â2?¿è.ewS¿ë@˜Á­^ó¿ìKt½Âè¿Ù¿†ÞV&AGNbcuPMN J1352-2745?ïâìàNÅò?`<JDR?VHÛrXð?L»-a×4?aî²éQ|?X‰_3ôþŠ?ï­ö(Cs¦?€e™ýŒœ'?aa}@ðýƒ?fâ"qϳ*?€*¬ý=?yX™#m9?ïtc]X±Ù?'ù>©ã°•?n#2"¼·ï?iFeތØã?‹^\LeÀ?2YÊóÂÿ?ï<R0è?pãª'm?xï^w¥˜?X'9ça?'9åØK+?mñÍÛ?ïÆ°?‰"?qå‹Òb?eÏË;Ôu?]Ñ\òÚ?r "<3¼?i¦ WiÄx?ïïË÷² ?–}h5žrq?t¤¨L'(?z!§b?˜¸ÜkU'v?'­e™Ûàp?î¾\Šfî?'þY.;ôð?…l_%‰ºD?åŠ/,·?†äÕ
%?ŽQ5/	§?í]ÕSM?"¦w´¨¤á?–E\ÉÞå?}*˜ö¬¨>?®ÿÿ˙õI?šŸßöù†AGN4FGL J1353.0-4413?îá™9;NÏ@1D^=¢ø¾À9u –
À<ùée‰È@9€H9Ö@cZþSW–?²¹'©gB?°c¥kßÍ?ü6~â^.Š@õ¾]ž@È¿ä«KÞ$ãå¿Öì@Ûgo¿ãýMž"[¿âgT"*d¿äÌ~É3»¿ëZ0Íþ%4AGNbll3FGL J1353.1-4414PKS 1349-439?ïÕ‹U¼©?h§{bيg?N÷éع?C%Ø
·3?q¦;VUì­?dæ®?ï¼ú"±'€?{¶,S›_¤?\Z˜õ&T ?d"Dé3Û?zl`ƒÃ?tT~:
²?ï'ØPtÈ»?|°'Ë¡€ý?càˆ4Ò#?ebío3†l?†ÃsÊ·z©?w…Kì®
?ïSÅIB‰?l=Fs3(Î?}žšõ6:á?Y"½¨ËÈa?Œ?`NZ'.?eN>uˆL¨?ïªÞ–ßç?u°õã?`Ž6¢v?QIa9€%<?@v»9ѯ?rkÍÀª
?ï3²âüö?•â´ùC
Ì?u Ji'êô?‹Úb`Ð?"V÷³Ó'?:÷*vÿ™?îõµçáƒÇ?'šLëí®­?t–«ž˜ù?r»¶¯á°?œEVØð?€‡¨?°?î\y͘Ç?ˆ—÷×2C"?'®w>™Ñ?vøcÛýÛ? áSë°)ã?'†"iÁ*AGN4FGL J1353.2+3740?ìZ»ëS¸@RPñýÞ½À:øªÇ¿FÒÀ<ºjÖ7¯š@(YØ8À?þšþSW•é?ÑK,¹œn`?Å<EÖxó?ót1ËT&É@W9°$ö?ïù¿`}™¿ê:'¦.(¿á hUSïk¿ÒgC±Ý¿á¾Ÿ­¯Ñ¿ïÿå=†ô&AGNbllRGB J1353+376?ïÓLfÇ—?fð<b¹¸
?P0e˔·x?A"ÿ5³ Á?rM³'çP?dÑþì­Þb?ïÒ$ُd?t¿Â~¾m?CÕÅ
DÞ?Lœt&F?ã?trÚ¯È'?sbÚÀé/?ïG»eˬ?…åîך£]?g´‹p2®X?khòlJK?"èÀü¾?"‰¹_"5^?ï'þ…Š ³?d>'*?jö~Ê$ï«?K©2"ú¤&?"'¾ù´é*?b‡êàßU?ï¨ËƒÕÍ?}¾Yí\9g?ZRQž'®—?RV£5[ÏÝ?''ÔÇBæ?{†¿ü-?ïsÈ/•U#?Ž­&}èð?Z«ØAW–?a€	ê«U<?¸y	ªnk?Œ©™ŽSaÉ?î±Ô‡ðé{?'{_+e‡º?p³öl-?q˜5¸Àó?¢ÌTÞ§áH?'îÆsv­!?îÚÀ~gå?uêOüm?{s¸H´?id 
Èk?ÊýI)Z;?€n•‹¢HAGN4FGL J1353.3+1434¿ïÿ©\ÉôD@Q¸«`kz¢À9æÔø³À<e¹@þÍÑ@ !‡å<@üæb I?²˜8_[Éï?TrÈkáqí?¥(æ~#ÇZ@
»Õ§ç»?ïüü_·u£¿ä}üàeÛÒ¿ä,u©ÐH'¿â0›©>R¿äa߃ˆ¶¿éfj˜$N"AGNbll3FGL J1353.2+1435OP 186?ï}ê,•Eˆ?­¶h£«¶ë?MY/K¬?]$¢-ˆ?§?Ž¯áí`å?­B"Fç"%?ïޚ(¤}½?q'È)ýçæ?C1aÊ2$?Nh¨+GÄ?l¢
ü
OD?nz¬–»á ?ïr,uÝZ?"®pS?¼/?WüyûQ$?`÷ÊKC}?œñòÊXz?"‰ÜÐ4',?ïÝEØsÁe?OͦÙ&`ê?T3œÂ{?8(f͗!?h²
âùU]?J˜ñ‹ˆ?ï™i
'?€EÒË~?PŸ‰ó1Y?Qß
gTÍ?‡«4{ѕ[?ŒR-·WÌn?ïÀ‹t?'y=+û¨?NþíËeê¤?[JŠ³à?Š 
°‰Õi?Õ¿'ZBÝ?îbæ;€++?žN䳁ã?b—SÖü?fRhök.0?¨°RÚÍ©\?žG¥*þM§?ïŸd)^?oBá=%‡?mÄ$ÞäÙ?XI13îå?€ÂĦÅÊ?i,™ãÙÀ9AGN4FGL J1353.4+5600?æìï'HKý@M…çÀn¹À;A£[º:úÀ<ºŠ´úH0@ä4µê2@‡"ƒ¸†Å?ÃÙ¹"ÆxË¿"šmÚÎî?Ñɋ¤¹]Y@3=gµj¿ïî5'˜Ì?ïíÜ|m8è¿çl]Á|6²¿äXb—¤Í¿àƁŠY5¿Áè›_lw"AGNbllRX J1353.4+5601?ïÞcøN8?`>s@Þÿ??CU5ó…Æ?4ÀÐ7,4?lÇ¢¥ã¨&?^_ÚÅ®¬n?ïڅnX<?né΋MR?AóÀäÿÇ5?KT[ºo¯?p~ЪÑÊ?jo>Ú	æÿ?ïi
H`õl?')Õú8Žé?d–î®ã™?ix
aZÂ?KÙ‡0?€‹<á"#s?ïÄB@'ž'?[¥¶8XÝw?_eßb–?F0K™9ì?vÆR«ç¯?[2å]Lï??ï·| Àr?ra½?Sc®ê#u×?F¼)ȦÔ?içM§?qÃokž»?ïg'‰ª¹?ˆ'›}²N?T%AÜWÿý?`Tè:j¢Ê?‰¡sV¯Ç?…æs?|g'?îÙò×gI?Œ/wÑm§k?p5kŸÈÌ$?mò
̝4&? hÓ]r'h?‰lږ0zé?ïL<0Ýv?yF ÷$šÚ?vdg×Tc"?hõe¼*9Ñ?ßcëFfj?xj^MR@,AGN4FGL J1353.6-6640?ÙdY›Ò¯À)×⪄£À9þ…¬|ËÀ;ϏÁàá@ ÅÏþ¨0?þÚvÙ{0ù?¬ï܂ˆ—$?_¤ßʚ1?µEÀÂ}i@Èm`€žK?ïÿwD;Ï¿Ú×.(\¿â³y…'¿à?€³ï†5¿×ȱil«¿Ø"<z¯ž"AGNbll3FGL J1353.5-66401RXS J135341.1-664002?é§Î¢\?¾œæ2×÷+?kóà÷vû|?`ݦKr1?ÈôC¼ ã?¾qÁg­¨?ënÉ*?·¶ÑÛüÖÛ?[&sšÌ'?e^Lhò³j?ÂZ¦Ðl?·u/Eהk?ìøyç¼?¥÷´6eÞ$?€Žq±–æ?y²Ò"U'i?½	Dn¼C?¥˜¡Æ£Ÿ?î‹@:ƒ?ŠC-»ÊÒê?'įÏÀaú?cæw½Ù™T?ª.ËT´Ü?ˆ:_'Û¼?âh
îä?njW±í£\?~ZH›YH*?rŸÅ¤WÂC?Ú¶'µžÕ:?Ǎ'´˜?äÂð0QØ?ÇäK¦iD?cN§Ë¾o?uå¹:CQÊ?ÖS'PGá?ÇÏO´¤Ò?çÚ¼F=|?°b¹WŒõ?Šc8‹A$(?r‰½2ð?ÎîÜ×å?°T—¢Ã?ëDՑ0XQ?£¦jç™E¦?—‰š=Æn–?nÄþÕ&?¿öìäwìÔ?¢€Õg ÄAGN4FGL J1353.7-3936¿±/I c¤@5±¶€Z-sÀ;Ȃ—õT«À<ØøγVÚ@"´à®ø{?öĺ|h?Ú&Á HàD?Ú{¤üۈ?úµÄ}î@ø‰*
Àx?£!¼'õ
¿ïü˜!I{Ê?ïþ±¶ÆÑ
¿£×*©»¿Ñ³œ¾ß¤¿Ú€~ÀzYAGNbcuNVSS J135345-393711?ïxÚó½7À?†<€Îlk*?]Öw=÷£å?P¥¾MՌ>?ŽtDo­?…I"äý.å?ïJÇ%1ׂ?"O4ñ¬?ojtɛ¶ö?v/Ý
Ä?'¹Ì¹tâ?'h™¥?îŽfúNÕ?¢eè[µP?bՒà—*ç?^r=w>VÑ?®¹Àd5i?¢UX\nˆ!?¡af?"Ô¸W'?SO¾'Ks?CMR>-ú)?¥;gô«Å?"™x_ØŹ?îӏ͊Y?Ÿ"›¯u-g?pÂø25B;?kYe…e? ¶çÿ b?"¯0Ö?î€^úâ3ç?©±˜Pߺ'?wÑý‰¾:O?ŠeÇ㌊p?¤ÿП)Å?§?".¶<a?ì9c®¦2?«$:ÇÒ/?d
#BÅåa?gVö§&Î?½"'rÑÁ?«\ô?ì/3Þ²?£©¤ów­ø?a%
 >?`òߍDÓ?¿_T=2Õ?£˜gî»YêAGN4FGL J1354.2+6934¿Ö]s±†(@GJ»˜Çâ'À;9‹n]«­À<⟍Ï`ü@ëëêÊ8É@Ñ·Xâ?ÕlEãäìS?Ó`;^ÐÅÖ?ù|ÙÚÒI?ý€ÌC:?ïû:~+)$¿ç]=B€®¿á¾-,ˆõ¿çiÆ×p•¿ïÓ9ÎWçH¿ï*èáÖIAGNbcu87GB 135252.8+694626?îîÉp!?š÷š{¢ÕÜ?€4}èè|?y|_¤×´?£¹ÑsTÕR?—Ä메‹?îBB~:ÿ—?Ÿ-ߝp$?"œ6¢–|à?Ï`Õº?¢
¼Ç•,,?—"Ó—üy?í…Ic a?#ë)qÊ?—"®´o$?ŽT·ˆ*c?«äd
¸e?–ãq­V	Ù?ížJŒ|`à?Ž"¨q?£?ŸøåL?"ÓÈæúz¤?¢ü—e%¸?€ÇôñK?ì"+‰yC–?­ë–0#s?'õ÷ØV?‡3±L,˜?¶é^+:?«ì,ZRÇ?ët8´?¶"ÂdA‡°?§ÔàúM°Ú?©êJuL¼?¸sÎükr?¯ ó¨Û`?ëޙ.uðX?¤âzG¿"F? êË]³zÆ?':­]Ã@?¸•ÐÞÀšX?¢™˜µ•?긊c?¤	Píę?°Wo]Èív? Àï4[?¹èlP
Yu?œªGj6zqAGN4FGL J1354.3-0206?ï`´åi@L‡çB™Ø"À:bÑÜFwÀ<+Z§ƒ@;ç¿ÂMB@\àž:é
?Ғ	†gä?á%'`À48@×WŸúë@¤R˜(U?àÒt¬zFî¿ák™v^+/¿é•1 6ç¿ï¬ÖøŸ¹n?ÚUÛ>T¤r¿îû¶úÓpUAGNfsrqPKS 1351-018?îä¬y?ª\ˆ¬jB?‰ï0ã?J8</Ò?§•÷ái
1?¦'4#þIã?ïÛ\vgT?¢˜™¶Â@Ï?†A=ãlQ?˜WiŽÞ†?"cõ≑S?'€œ\ÞY?ë&R|F?§í¤(¦?¯¸Z±¹?œ6t×?·Lò†,Æ?£˜°Ü?ï:uJœ#?ƒ'—‡qª?g°¦<þí?``;ä¨þ?•»Aûq&¾?''Äd#»#?ëǕâb?¹´´A î?ž@|0¢ì? ±öo£õë?º38 `?¶~—"B‹p?íg #\·¢?¸­sè›d"? ¬ÞmN±?¯¿Œri©è?¨Ùa1WÃ?ªñÛ̅Y?æ±qrðÆ?±ÇIÍíü?¾Ê+éÔ?¦eAÎ+œ'?ÅÕ$®¤Ý^?«2%Dœ·è?íg}¢Ã?£ÙõxiR'?Æôcô*?"Hœn8¬j?²‹4_AÔÃ?¢I‡¥©±åAGN4FGL J1354.4+3707¿—í<¬ú7@RWRÁmóùÀ:‡à	Às"À<"Ûá<ÆZ@ãZÅô@"?ÿ¾•·ŒÉ§?¿˜kàè|p?£\Ðeˆšï?ås|>ió@¦IÐÙvÔ¿ÔWQ?ãšÅ?ì¤'D`'¿âƒ''g›ñ¿áÞSÝͦ¿ÜÂ÷¡aº¿à蒀u±2AGNbll3FGL J1354.5+3705NVSS J135426+370654?ïØ·'ºœ?_•°±YC?R¸úÆML?B¯0#V?mëðP-'?Z+[§1cû?ïÉ´2»ØÍ?z*0àZŽ»?Q0‰Î¼Ž?['uß.?vÙÆDo^?uT Œ™(J?ï…fõéŒÝ?t0Âcg‰?b«*" à?aƒÏy@°å?‰û€láz?q_'­YN'?ï*rß	?t	|p]õ?ˆT0âS¥L?jŽRð¾º?'™8go?nZlôp?ï±B;J1?q«0|•îç?e¤øµpŠ?Ze‹
7Îè?|Œfˆ6Ü?já¿S‡#?ïIdpu'…?• 	§÷êÙ?i)T	ÞûI?qæÎÒrÀr?"®Gtµhë?'ûáûA±$?ï+3"Iß{?€>¹š5¹?k6¶ž{w?aáJ¸Ôä?—2ÄùCÎ6?}˜Wk?í¸€/÷O¾?TF'$y3?œñ\Š£?††~ƒ•V?¥ÿyp¤ðÊ?‡VÜhsAGN4FGL J1354.7+0623¿é©ù@ѵ@PøôsÀ;EÖÌ*žÀ<¬Kä ÷@ 1´XÛ?þÐßìdAÉ?×¼.Ääv?¿L'Jò—?ì°ç~~á@†,ÞZi?뛽˨	Ÿ¿ä	"ˆÁB¿à™"º\‡À¿ÐÈøÂI?¿åøžï!‹¿ïÿø]Ê5™AGNbllNVSS J135444+062249?ïéeó†[?j†¼ù/Ø?;µu7pÅ?.û˜,f?c$Op ¾'?jY¤?ïµT†•?yrcª¶?Qu¨0ß¾?S-ēS=š?€'5Þ8xû?wnz')?ïhªñ°²?ƒMŒš–\?ZâTj…ÅÕ?BÚ¸‰ö8ü?'NÅ^93b?ƒ!%³ÓŠŒ?ï4fÔËHé?tz‰A0o?kÖÁä*¨E?P›—'Ôï?•øM%šÙ?sO6´W?ïÚy¨Yó3?bÔÑÝéŽÔ?F	]»‹Ë•?=rúæëýÚ?pƹ4?a
ûeªì?ïGù›YY°?'†'œš-}?_p±¸†.,?eÇèÅzk?•	ÁxD…!?uÁš‹ÿJ?îàìÞ~ê°?ùWȨu·?g@,׀°A?`ö£Š‡ §? }/Mòèp?H1ÆAZx?íÄSoÏ×Õ?'ÿi1eá?yÞ5þC‰?pP§öEx?°?!u?È¾ÐSͯAGN4FGL J1354.8-1041?ìÁë²Áó@H•žbV6mÀ9y˜éåÀ;ÿä[^Ëg@n¥ÇzS@*¬azŠ?³Æÿ> 4ú?ǚ}DNc@#»@³Nw@›°´é+R?ºªÅ»ám¿âÈ}}`Þ¿äù— ¢‰¿é[ibš)¿æ1]À¥w¿ç± @Ò®
AGNfsrq3FGL J1355.0-1044PKS 1352-104?ïå;î‡?a.ÜZ3%:?YNùž @Ú?Te»?Œ€?\"Wö/ ?T^"•^¼?ïٓœÕcI?o!k4¬Z?F"îø[•?PEVÔ֏!?pdÛ0ìs?iNÐõÖ"?ïd8zsl?‰Ýl^ gl?y®x'ÿœ¼?}.°grr<?Š¾#:ƒ?ƒsÎûns?ïÜÙª€Ç'?QS4'|AŒ?PnÁ]¾±0?6YH³²{f?jîõ±nh?Lgê"ψ?ïÔx¹¹þ?kG!£°?`wl}i¨´?VàØ5¡Mž?kƒ§à^?c'3"ƒn?ïrR‡%<"?"»®ü´m?^íz¯X#¬?iÁŽ˜›*0?®ÑO˜Ž?"Ge*X?îº6xÂ7?™*"€Ï?ŠüH¥> ?‰;·ÙN$ ?›;§u}Å?"°'g²r­?ï›ÝfM?p³‹¾}¿?gƒ<€Ø?T·*q́?ƒ'×9¬+ê?k\a·Î`'AGN4FGL J1356.2-1726¿êV³œ`Y˜@E]ȟ@¢‡À;ùÿ4þåÀ=2Pµ$:@ @ԋ2"½?øóy	YÂ?×[	T<˜?íGâb
a-@
VŸ¸g?ýø8RÌ+¿ëÿÝe¡D‰¿ØàEš¾Ý¡¿Â¢HڏX¿°¹€AS²¿êêË»TÕD¿ðAGNagnPKS B1353-171?ê¥OÁoˆ?¸,Îâs?¸à«Mß6?­¬x?=ì?·*eÌf	?­t[ëåÏ?èjXmK?Ãh(ƦJ¶?čÃ;mX?Á6ãÄ™€?´ª!êå¯?©I¸¨Ý?é6&W­'?²~à·ü‹J?·L‰t?¥ÿÊìq®?¿ÂHB®v?«[/OÉ¢é?çŒQ‡‡?­²cÕΏ?ÃÐ\Eȃ‰?¬)]ÄǾÈ?¿+â¼´?›ÍpÐfy ?ç#-?½jÙñ+.‹?Á&–JbWl?³œ>dìH?¾5óVú7¿?³.T%?V?àäÃT4¢?̎¶bc]¯?Ô6pËó?ÌÖR²÷?Äp+Gh?µ¬D¦FR?å'¡Ê.?¸nx¶jÎ?ÂVêxë_p?±fï~K·?É8¯|wÖ?´Éì˜{(Ä?ÝP=L3+É?¹ÕD"X-­?Ñ-·üd%?»Ë˜fÙS?тªÐp?² 'š8ÇAGN4FGL J1357.1+1921¿îÒ[Í0Iõ@RBä¸{ÜðÀ:?
€Œ'ZÀ<^gpQ¢@‹íi>]@ý‹{ɤú?¼¸•!(³l?Ž3Š4æ€l?Ç⧋P@
6҇v×M¿ãv֋'oڿ䜝Öj/¿ë SÇþ0ó¿åèe¯‡A¨¿ð?ðAGNfsrq4C +19.44?ïö]p…­?OÙI+ýšŒ?Avx‹?FëÁWº{†?EnêJ¥ÈÇ?B&›¿–«?ïәºÑ¢Ÿ?}´3Kxx´?ET òº•?RŸKw´?sˆŠ\ £ÿ?{ᯊ­$´?ï™
ZD?˜»§þŠ?lÌÝRÎ2?vfê²^Á?'ˆÃœ?vl }aŸ>?ïñ©/[.Ç?AÂêq:l ?AMÈ,µt?-Â2Ó»S?T¼è=='?;a&õj'ç?ïñ>ß8à?V³3›Rt?IPLÓZöÈ?GÜ@PÞ¯ð?PÚåŸÜž?P÷͉d²ý?ïuº&ôâ?—¤p¡Î}?Xíz…lçæ?g_€[>›ð?sÇ&~"?•ý6ó#?ïFU"Ÿ?…UâŒ\N?rËæÀåH$?uQÃZGö?''SÙ{Cß?'Àåø¶?ïʒ2«µ?h<ÿé'º?aÅuØÛ·?T'÷l	Ë?r)ܦ>W¦?c"h»xb"AGN4FGL J1357.5+0127¿ÓŸ2ü'ÉW@Méä¼­šØÀ:/½¦îíÀ<V8‰´IH@Ú;ƒd@ü wnÌ?Àx^ õ-"?Ã%›Åî·@oPóÇ
?ÿî>¯h7ø¿ëïþ€#&?ï	þ¡[.û¿ãOˆžŸ'Ø¿ä‰]aZ
¿âàsr¾c}¿ïÿªÅÝðAGNbll3FGL J1357.5+0125RX J1357.6+0128?ïrrAw)é?~*£ݐ+?ua%?j…,ÁQ^	?ˆ'(.N¬?wK\‰À¡?ïIQ`M{?›±º›É~÷?‡;º‰N)?Ž¡\:üEÚ?"9SïÒqŽ?Ž4²_]M?îýxCç(?ŒŒÈ…'b>?€Õ}?~ÒjC‰Ma?—æo''6Á?…ïâU«_?ì~‰uŠÌ?'.ªuO†}?¯@Þ,ö¢?ŽÌ«#`«‡?¨ÖŠ{C˜0?Á8žïŠ?îmñzs¨?–̐"2Á?•ÆV×vK?Œ}þ–E²?"?~¢?nUDÁU>?ìÕ]v—{?µž=HYê?¡ÿÆ͘õf?¨E9ðç‰<?°Wù­ì¼ö?©hÈÆvÕ?íÓånÈúI?œÝU
goÍ?"A†/
ƒ?vkußþ?© àÌ
S2?•+€œÅ	?èFft[Ð?¤ô¸Ö×°?ÀØhL†?¤º`õŸe?¼©ÔñV?˜%{ ÆoÍAGN4FGL J1358.1+7642?ÉLÅ!ÿüq@CãŒCoÁYÀ:ítãìÀ<¯¾5ZTà@ŠÍ©ìx@¤%t:?´,Ù&ø?¦ÒU¢ÉÄ?ðjâF±•9@wûmŸÙ?å_¢!¨q¿ß›j$ÎA¿äýýâŽl¿ãÙwÕúrø¿êþMxX×2¿ïÿŒýÿʦAGNfsrq3FGL J1357.6+7643S5 1357+76?ïÊ+Ýø?­	"C|ã?SŒà ¦Ç?~¡ŽÃõ?vÙc`.?©7@@²?ïÜÒ@ £Ü?pJ!{k¬Z?C¢ì:+?Pǂeîlë?nE=
õ>í?j`²l)A?祥wn?~Hn¨Ýó?dY]x…ê'?mö•¿`¥Í?€ç÷ï:?zBÚR-·?ïñÚÔ³‡=?=!²¢Éßµ?KqBÊê®?0Á4LDzV?M#kSGU'?3gÒítßû?ïÅ+Øä
?'ì8ω¨{?\~¨?ös?jp-ýxÃ	?vJi÷½«»?f®ÞðÓÍ?ï˜Éê3(æ?…ÊDš)Z™?SÚVîïÉ?a|[¸v?‡R:›˜ˆ‰?ƒ(ƒžYî›?ïa!κkT?‡"nðN?oÊxÌ©î$?v×	û .3?Äî+ùj?ƒøN[.Ü+?ïÙà>¿j?]E߆+‰?bö'ÙG¸[?O›šE~ï?c)™õ;®:?Rj{ˆ/c™AGN4FGL J1358.9-0703¿àò$±Kx@J
At>–>À;Ž²‹Øæ·À=þæ$Œ§@&þTb`?ù(
Jk^?×ÉÔ_hEd?çN—rwì¡@Æþ÷ÂCÝ@mI%7òá?ï­àx{;á¿èÈ¿AHõ'¿Æj!´Û"¿Ä³w¼$3¿íQÖ¤¿ì‰pÃõ8AGNbcuNVSS J135850-070403?íHïg¨Ó?ªÂùÇÿ?¢ý$Ú/)ò?˜ÎŸ$W?¨sê
žzß?£Î…Ñ¿™?íÒjéWòÛ?«×Ž™KÆ?ž²1X!0%?¢œ‹‡S?£€8ÁßÖ6?›">?ì€â̦?¥V	ÐB¶?£ÙZþ?–<c&£ªU?²KrîTÊ? SÙ9ûJû?í%k/+š@?'Ê"¥i?¤°l™Ü4Ÿ?Œæ±•ÝÏ?¨øàtF\?†)ÙäÆ?ê¼n\¶?º¼õœØF?±Éiû»/"?¥åÌgé¯?¸S%¨òW??·ÉE¯'Çv?긭Àt?¼\ÖÅ?±LV¡2¦W?³f—ÓP?¸î;YãÅ9?°Ìœ©@?é\gïþU0?²Šf<¶Cè?°â´hóv"? 'x®§½?Â
±÷?®	-êã§ô?éo…ãž?«;u°‡ü÷?´€"_lí?¦Lùº¸ðn?Áø8òv?¢å4Âg^­AGN4FGL J1359.1+5544¿æätÜÿR@Mq%F
¦LÀ9¢x>Õþ¥À<Q¸ÕŸf@v$4Õk@ã¼ûžqp?­7¿^û
'?¼û•0©@@c¦@q	@Å?à?Æ?¿Ô÷íwg?ª¿ã=]º¿ä<Ž@ @¿è«þ +ï¿ì ©¡Nš¿ßáŒAÂB/AGNfsrq3FGL J1359.0+554487GB 135720.6+555936?ï‰y]äâ˜?ªƒ/]™?i‹ý]é@?‡±T/Þé%?‡>©,5rf?¤mÁ…;¬?️6ùc?|Mî¤Ó©t?\£¡tuC?eœ%(CA$?||›I…?t½¶RŽ¢ƒ?ï|¦B¹&ì?†9õB's?yDg¸žá
?©?•Fl¯?"4;"-&J?~ܚ¹>üp?ï¶T6§Ë¥?]}ƒE'®à?pÏà°û?RMaéDHÐ?t²%?Sƒ9Ëõ¬«?ï
B¢?¬š`*A"ö?xY9Oc·?2Uü©†?˜WžŒ†ø?¥g±uE‹×?ï'ãe"Ç?–?¸(…B:?mR£ßðJh?uàGBuÐ?—YJ'L,Ï?"ÈBÞÓ³¼?îë¢0È0?•ÓÂð?ˆîB'ê@?‰Øè‹hŠ?–¿}únÖ?7.´V/ù?ïÃ¥å5?¨AÅJ·?Š¿ˆõ>À?u€‡±Þ£?ŽŸaðæ?uµ%øæÈAGN4FGL J1359.1-1152?ÔOp³ÞÌ@GՊ"-QrÀ;ًŸeÀ<ÏÅ'iú@#"ß³Y^@?çK¶ý'¢1?æZŸRk2?ã÷{a .?øȃweR@ùi'é÷Ö?ïñZJÏ1¿ÍÏã؂µ¿ãßIÈ¿äøRAkZA¿ÿâm•Q?ÊxýrñºAGNbcu2MASS J13592131-1150440?ï€.fÎHÖ?ŠûX}$?hÌÿqjž?]D[®UÃ?‰î3í¹?‰oºœe3?îÄ[gëÝÅ?¬ŸŽ®·–?ƒ/¬×îÏ?§Æ—"?Ü¼Ÿ|3b?¨~g–ÀŠð?î@ú°ž?ší#8Ò?~lx'ýŒø?€‡-•ÁF'?¨"ÏÒƒ?˜ •PF@?ì{+'ï?§x4ž\å?`N*õYÛ?aeùC«?»¡–Nq¹<?§\''9'¹?ï"ñ'ÊÜ?•¿F…P?{QC˜0?rYºhìˆ?—G`?D‰S?'þ9¯¸»?ímœW˜?·Éâ¼T,ô?Žo{~t¦Ð?¡¦šÏrÆ%?¯]GaqÄ?´Í¶W,œ?íXÖ
c0Q? xv	KÍ?"°dS e?êÀ¼J?²£C)k?Ÿ>#£´Ã?æ>Ý­½	ƒ?ÀTÀ±?f3ñ5ð!p?|$õTúª?ÓUÜÁó'?À­Êå'HAGN4FGL J1359.4+0202?ì<'
öló@N'¼U†DÀ:"R:_w_À<Qhª
…@ ¿'țæ@]¨!ò™?Ëæ	³õ?Ï؎!yd@¿2½ÂmÎ@Z½Ä³Ï?ïÎÃè!¼é¿ä…Õ"ܤ¿çuM‰öŽ¿áÉ/ß@¾¿ïÿ×,uª?æ9i"ƒb¡AGNfsrq3FGL J1359.2+0204PKS 1356+022?ïÏM/*1y?j0ùšæ??VTW¸F?HͽkÉü?rÄR¤ðiO?f¥Êmä—i?ï¯Mà™Ä?€›dýµå?[8©0¼¾"?bfd—XF?€ÓT³s#?{Εd"A?ïM}ƒ'V?†Ã³=¶m?wXF…¥çË?y
`xˆi?z=ú/³+?W³3°?ï¡a'À\Q?fñ®í·~?l"etóK?R±+Ù½#?€¢6‡	ÎÓ?aâÎdÿ'?ï‹<Nj ?€Ñݑ˜Ô°?hhЈÌøV?[œîj°½Ã?‡¸m/é?~Dò[Ó>š?ï6Óá¾÷L?˜ ÑkH÷‹?k›ó悺?yíCãû)¼?•²oW[?"WÔ­_×Ó?Ï?"Ñ ¢ö…E?‡Cù3p
x?ƒ•¿NÇÔº?¡ÏôZÁ~?Žü)áĹU?€Q–m?ˆÉHãVy?†Næ(¼­?sÅhB÷-ï?ž'(‹OÙü?"kb[`?-AGN4FGL J1359.7+4012¿…ø͞¾M@Q°–»™À:V²w¶ðÂÀ<|J{NTø@^VòU'@ž[BEõ®?ÂZCBð?О饴¦@	<J@•òE@G,íHî0?ï÷6Íòfº¿Ù«"}¨¢K¿è>Æ¿—…¿ê~€¿ê'•¿¿ïü€s,óAGNfsrq87GB 135731.7+402612?ï«)ƒôV?xt¢—V·´?gâüx±ÎŒ?]ÝK¹&¨¼?~yÀ#.ÍÛ?u5C¾z?ïÈ¡^Vnï?xÈcâúŸè?V®ÊX«I9?cäÅI՝?vž!d?qöoñG?îèÏûç}¹?'"ª{Žá?‡Á·æxÔÚ?†oîÒ•?—$'‹¬g?‹Q›5øuÍ?ï½¢â1|¿?Z1VÓâ?o-Šâz"?RÁ"™&2?q«x¢W‹?P¥kP…Or?ï/@tå/D?•E-Ÿ±?u¹!†!ì‰?oçáùIJ~?"©©Ù~U?"w…ÿ{#L?ïU–õÐQ<?"GSÓF '?m3!&»?‹Ê†Ÿz?'¦±*?_t2@"Ò?íÿߥ±CÉ?žaå$?– @V 7?§è/âm^?¤òõQX?–ŒuÎ÷?ïMa×­ÈÈ?y«$+=?ƒ×­Ž""?oìP?okó?ˆÐsX8ç'?pð'ä®<AGN4FGL J1359.8-3746¿îÀÞÿ¡­²@7&=_ÜßjÀ9…/…(ÉÀ<¨a³y@ºYÀ7@"ý°šg?¬ªþå´á¿ 3ÀîÈ?ó@YÂ5g@N}âÝ?â{8 Z}û¿àr·!ê¶m¿årÚ/­m¿Úx›)ñì¿ÚÄGÃ
0j¿åÅYa›AGNbll3FGL J1359.9-3746PMN J1359-3746?ïÔ `â]?«²º] ¦ð?GPÉO¼ß"?wýëK'£z?sքϼ¥?¨³8êìÃC?ïá|£®_=?o«}uåH
?Bíü ³[/?P¸êy|^ó?iÇÝ¥Ðþ?il÷ýž?ï±w˂c·?y+ÅY$¯C?R½"À?Uú*èO?Jl­Î¿÷?xA‡*q¥?ï}4øÉð?f™˜-
"?_Ïå"Lj?=MÎ]?ˆ>˜Ñyƒ?eÆaèÄb?ïÆ´¦ª'?«KŽAùT?RQ¦K
Ük?eL»Oæ?xCRý™?ˆÙwìñf?ï›W¨n¯Ç?šóŸ
e²ü?V"‰§¹ð?c‡tè-%%?†W¤µ42j?šS˜ÜÄâT?ïk?wë]?"po
ZÚ¸?]J]'îŽð?aÆLԑ·?ÃkJüw?ƒ»ŒÐ¶ÐÝ?î¯Ä_¯¬Å?"#&…+Ì­?x¤­¾Ó†™?_˜ôe'Ší?¡ï$O:†×?ƒ¦®dà´öAGN4FGL J1400.2-4010¿í¤ÃÓÌ<Ñ@4Ðù;À oÀ;ñ՚ѨÀ<Š¹æ@;Y@ ÐXz•rn?ÿ"<jÿR?ÉèxyäG"?³ÿè¿,âG?ä¢ÿñ?ïäOþ΅<¿Ø—"{ªñ0¿Úki¦Wî?ÞçÖyô¹¿äh M¼¿Úd¢Qy¿á'Y
]QAGNbll2MASS J14002208-4008235?ïýðu`?PCèÇu?S-€0÷?UDx3O.-?~)ÿ»?Ž÷L'Jò˜?gnµQ?£¶$v¤CŽ?…ÐDÇn'?Š…Í»³j"? ƒ˜Z½+h?¡Mc+»ž?ï	ø´²#Ô?ŒÚPaúî_?{œ¸;©üú?~òÉ}ŽS?—Ù»a"C5?‡žm´{²?ëk†GŸ?œŒ¿bù@ë?'ÒŸÝqù?—&˜Gû?ÁýëlŽã?›=ó1Ž¹?î$é÷Þ|?ŸqÁuH?f┓ÚÄ?_âÃv
U°?¤¿ˆܼ÷?žu—''Y?ì[by^¤?¹²T{'W^?œ[a¯Û?û?¬
l·ÿ¯O?¶ÉHye?´£ÏÍw?î$ÖhW?—¦~žGý?…±0:«M?";@Ö.U?¨FR…ïÿ¾?"6™jæ?äwÕZv)c?°CĹ5žÑ?žØ"ò"P?•GÂ.ãŸ?Õ"Ì"†?°9R…S©…AGN4FGL J1400.6-5605¿°;hÙÐð@õ†_*2À9 syt`$À;¥›/›Ï@§ÍŸ°‰ö@
œ \–Ú?µ@1ôCß(?·\<ìÅe¥@,Gõb@i‡-0e?ïÿúŒ—Ó¿å:ú!™­¼¿è.[}T>œ¿äǸ@MÍé¿åyÁg‰&¿ïÿܞüÚÝAGNbcu3FGL J1400.7-5605PMN J1400-5605?ÅEç7?'|œÐßÉ?>s÷¡jt9?4=?Mˆ?‰®ð,ž%?'=ÇoðoÁ?îçM¤Œ£?¢C±·på³?Thðol\
?d÷¯:õ@? çæ±3ðò?¡ž(ñõU?înOÛN^¢?–—+8¦?t9?eÀT?xô–&ò?¦š;!‹_?•ï{†/ÅÆ?ïj‡S#œ?i5—U}x?f{ƒ#vÌ?CÉÚ4ìä?¿Jg´•?g¸–‡ßéz?îÇ#å@?¢x5Wã?Pp™æ<S?Lô6†Äf·?£
‡‹Þ?¢4¦ãŸ›=?í:®%•?µXåâÄò?jcüB­c?~ZD["ú?µWrþÉJì?´éàþ?íä#søu?g¹~¯?ƒQg*£n?ƒÏnx'½¤?¬õ9lLT?šu{ÞñÞ?îF²Y·‰ø?‡ý{×_[?ƒ,¾š	B?gªµL‡Õè?¦ÉªÀsÓ*?…ڐ¦pAGN4FGL J1401.1-3717¿èuehd˜@7†Qm°ÝƒÀ:ˆWUQk-À<T"ÿ®¡i@ ÆK¢ë§Ù?ýJm\#íE?ѽH WÎÉ?»®ÛJ>´?ìÆÝ¿¹=ú@©ùŸ"®ž¿äp]€c½•¿äÐvH¿æ•§œ'œ¿È/Š1FÉé¿Ýê …0«ï¿âÞë}'üAGNbcuNVSS J140113-371757?ïʬÜ
ÿ¿?'pŠ/Üû
?>ÚÒì‰_?A¿'Þz:Ç?x»ä±Ìà?cÀ±>?ï¦?ÎæÇ9?€Ûp‹l©?X"'œ²"?^üpé`?ƒ]‰Çä5—?}ƒËS‰j¦?ïaӜʦ'?}œˆ¶AJñ?b1ò¾;v?]†ƒã¸?'N–ýù?{>m¥ª1?î˜DÕrã?`Œ¿¹ç^?li¨ä[?S"\x"Ö©?¤»ªŽÕ"?~Øeµ¦€?ï'6q¬?€ÄýśÂ?Ià†»°7ë?;ð}=pÒ?Š©ì¦p'?€FˆVÑu
?ïC'Ð!–?ž%Fï$Pò?n¹àtJÞ?w̳HÔ?œko@¨Ý?›Ö^–ÅF?0zFB?áI5ÇðÂ?q ,T:?gñÎݝÓY?¥q÷š?çHˌ5?ìq—á¢a?›?¥ OE?|2§²Û?nš‰k<¦²?½ùHŅt?šð+'#/dAGN4FGL J1401.2-0915¿í°òÚ0@@Hïâ£Î¦ÂÀ:¢nÚ©.bÀ<''¤{u@Í>¿‰È?ÿæ҂s"?ƪ4Üօ2?ɗ(¦w!?þó(ýOL@ë8[犿ìî`e›eL?ï÷`Æu¿äò–UAzõ¿ÜPj{žÝ¿ë±Èd?¹w?§ŠÈñAGNfsrqPKS B1358-090?îĺۙÕe?'úࣜ¼_?†‰Ì³QšŠ?}âdÃg?œ#¾;³Œ?Œ(IyÖ?ïŸEŸ¾Ä?'~ƒÜ$?eøVÃz ?k–A¯´£?'êÙï÷QŒ?xòc9×+f?îËðy?'=<­?}ʙhÄà?yû¶†`?Ÿ,Vï&É*?yú-]OI?îډºd¦"?xVø'v'?Ž
@8?lIºí$þ·?•¨(—g©÷?q"scÂÙ?ìùôFÓú?§M_§úò?MmåïZ,?'z]pç?°ÝPY$?¢ÿQ$"»?îÍ/l? ýž³¬6Í?y!އ?~ŒñÇV`ø? JPPè_?ž¿Œ­ÍÙ?ís†í;úy?¡»ñ'¹??°1E#I?‰Ì'h˜‡Û?°S܉`ïã?žØîšÝ#x?í1žøB
?'ôvVjè#?¢
××]n?…âÙ­oŠ?­'X9€hì?Œ'›'ȎAGN4FGL J1402.5-1827?Û?
#fÙË@D¡¥q"À:($5inYÀ<(]yWÚ²@
«)¹ã@·Mú^ÖO?½¢³ôŽ²¶?rõoÇýÊ?°öÌz—uÓ@¼"K̲ ?ì×aPQý¿æŽÛʖ'¿ã˜íl…¿çŌÁïÏ¿ïÿþó…õ?ïÿÚ €AGNbcuPMN J1402-1825?ï}'â¶Þ?›G«P«]?qöN"ª­?ƒb9Ú7µ?ƒ¥ŽÊ|ž3?'Ns	õ½«?{˜8?…s)«:¤î?fEþ`z?k|Ñ6ùò?‡@a€3Ó'?€¬9U˜?dØ><?–¯¤lD?Œl¦IêՂ?‹í`"üñ?žr 7kǼ?åHáɞ?~tt?jCn÷ÿà[?oÙà¡·ë?WÂ¥šñjá?'e(Dâô?bë¸iKD¸?îÇàxj
Õ?Þ•¥'ÖÁ?Šl97å?ˆ¯­*º\?™ûº×ô÷x?™q+Y-±?îïèØñô$?¤c¯?oCM®pؑ?xñglèå?ž{&H?£q;
Ès?ìÛóõõSî?¤Ä0Ø N:?_ÞY^v?•ë˜6d?±ÈhºÙ¤.? 'ò@°¼y?î°4NðD?‹7Ä!ŒŒ?‰ª·4p[C?yQÏ?$ ñûÑ?"—‡½ñAGN4FGL J1402.6+1600¿ë<aÿ	Ç@Q†	€²BÀ;-Ãք´À<­póˆ"@ …H~Éà?ÿj`Æê4½?Æx"%çEI¿{)øã0Zt?´¹øå¬Ã@™'6¿ïÿçÁŲ§?ïÿÿ>¹ú¿ëbrϏ¿ÅÚñéû%¿Õ0ÿ;ßÕ¿ç£ìòù‡AGNbll4C +16.39?îÊc«B…Ù?®'+Õüj?c¸ÿ—¥¦?k"µOöÂ?¢(ºìC˜?­¡lظ–Ê?ïâ‹ã
•?nduQ n?8[Êj±?DÁì>8?jh£mÝòó?jþïÍkwÚ?ïي³'?'TÖü8¹?n3ª#ÜQ?|Þ#éi'¢?›^j¶°•Y?ÒhÉì=n?ïÌ6UbÄ?]a†"Aˆ'?Nz»ÿ;\<?6û[ ¿?v*kd²D?\*¹¨oÛ?ï"ÿC?£þê®Äõ?d¦jøóL?o<'Ɉ?™J@Rñä?£3Ð.Y™I?ï¢sSE­?†ª'ŽÔÞX?HT÷Oø?StÛ·/Þh?…áŠ7똄?…Œù»&ãî?îxŠ\Ý?˜£ÝM-ó?wµâú‰v?ƒíÙ;`¢?¥€ÕU–ç?•œ3k¬W?ïc©yE?xù<ÀóI?eÎñ¨kôç?Xq÷Müw?äœ€Æ?v›j}ÄöBAGN4FGL J1402.6-3330?äŽêž;aL@;GÜ7£ÛÀ:˜) ã9÷À<kiA@®[®ýY@:9Å«â?Ò¸µ¾"N&?ïj-›C¾@	¼=h@[:@1mD&¤?f¾uœ¿¨»¶OùC¿î!3âÂ]¿â$A"HFÁ¿ïÿ••_x?ìѹÁ,Z§AGNfsrqPMN J1402-3334?ë­Ë™ŠÄÙ?Å~öÚV<?™sÕ2ê?Ÿs¬ å?¼4áýD3?ÄDŠà›r?ç«.'ÁÌ?ÌÉ5]Ÿ?Ë¢r¹¹}?ʇ|MOáa?±+a¬P' ?¨‹qÍG§ý?ë´ä9a0Ù?¦®ÂÇO«?©!}˜Ðÿ‰?œCN`¥š?µÈiiàu?¡é_³!‰?ë;Üï²?«*1¦Çþ§?À©^Ä£d?ªs,Ðô?š-'[þ²?ŽÎîœÌ›?ëÑfÌ£î?ÀïóòšU›?£¢Òkºü?¦9!ç^Þ?·¦;Æ-5?¾>¡Œ"\û?ݎÉ}¦¹?Ñi®®Ãf6?Ûóu`²Ñ?Ñyä8ŠqD?½v3;à?³É­ÖLb?éÛÄ"¯,?«Žvå?±ÕÏV¬ï? Þ‹»?¿Qä'Ž©?¦÷l0öZ?Þð}Š´[?ÃM,Ù|Þ?ÜÃužpK ?Ä
ҝ?±03^p0'?ž¶ùŠAGN4FGL J1403.4+4319¿æN©Œ3ˆ @Q
ðoiDgÀ<#01 3|À=$P%"õ@"…–VÄ?÷"Âkðê?×û .y?ÍЛ¹Y}u?ù´@€#@¼&‹*‡¿ïÿý{ÁA~¿ïÿÞ°ô)?ð¿âH+üÆ¿ÂDm'ºZ¿Âd5^±'2AGNbllNVSS J140319+432018?ëI&Ÿ¦ùÔ?Ç5הô:Ç?[˜ù·—«‹?Yæ1"f¾?¤3ŽÖO¶?Ç1"iS"3?ï"W=²Í?'9˜²{?c©Ï¯C¼¦?oºŠ³€S*?‰ÿ¼›ù±Œ?d¨Ö`e?ëÝ{DzÂÇ?ª·±­m©)?s*ŸßÛ}?|Ýá£ò®¡?¿âßÙR?ªt÷§×?ïRvª	(?|+˜mø;ž?@Jg·Rj?4O¦lÅ*+?•.Ôkâ<?|­N–¹?ê¬99;û?ÆÖÇ=|ôY?eÕYøÃ?f¬…wØ7'?Ä÷ÇP¥Î ?ÆÙà(À(?îˆÉ •?³TcjV·§?uþtãpz?†8#Ԏ½?¤³—cÖ ?²^´Ùό?êOh4ø?®v«µ©YP?xº8¯KÃ?V•«u?ÅüŽ4Ð[?®Ñfp"–?í°ÙJDØÞ?žËüa"–?K=j"BÇÜ?K‹ftó½?²BºÖÿKg?žÁÉ3q8ÖAGN4FGL J1404.8+6554¿œÊ÷ŒH@HÇé·¿ŽÀ:ªøf®‹À<Ž~(א@>Â?Ö?ýÕ%t-Ï?³š³Êó-à?«Æ¥bÇí·?ö7yU@
uèúÕÉ¡?ï÷€—9î¿á"†?IÁë¿ÙŸ:":½k¿Ü‹‰`'eC¿ás°0´Ó²¿Ùl#"¯¥AGNbll3FGL J1404.8+6554NVSS J140450+655428?ïöâ<)à?=^¬8ø?(j‹éÜ"u?•Ï%Ò?N\l+‰SC?9ԌèJô?ïàœyŒ¢ª?n›#ÍêK?A8dŸ¸©Â?K¾ä"‹ó?km¸ÿG?i¶oˏiü?ï¾{®L.,?nìûڔÎ?T‡VÉI?Tbz¬=?{ S<Ö´?l—Sk?ïÖ|‡v<®?L΁0ÿa?T@‹,Ž¿N?1´	ÂêA?oc3+Չ?J|pl»Fh?ïð܏@,ô?F¡â3$f?5ñ®,Ò9‡?#
~G$u	?XÊve÷Óy?D©56)!á?l.7²?‡±Ï¿r%Ÿ?SP{[S­c?^Ÿ&ì?ˆoՀ¡ß?…ò±%)W?ï—ãBsܵ?tËÝ`í«?]úž•Ï"?b•.K%?†Gے¶œ!?q%'*p ¹?}%'?n U¸Õ²A?hõDe4¸?N&*¨x?…–os?kÊ_u‹'QAGN4FGL J1404.8+0402¿ãZVb¸@N€ƒ§ŸíÀ9éF¹!õÀ<MÁ}ä1@…$1–¬@b"òB¨?³pbé"='?ƒ\³VGú?Ò'!,öX@Qî4P"˜?ïÂ.]á\§¿Ž¬)ò N¿æù­5WС¿Ò=ÉD6·¿æá	/Sª¢¿ÒºBUeAGNbll3FGL J1404.8+0401MS 1402.3+0416?ïÂúP
%ë?f¶çc-ù?N¶—#'X'?8vö€º'ã?z¬1Ž1¢?eV¨ê­¥ñ?ïÍ®ÝߪÜ?xšeŠ1?N'¼Žî›?X@Á˜¾‹Â?uV9…xH"?t;»iæ_?Åm¡³?uBÒ€D6?^æȝÿ_?V©RµA.?ˆ=u"GCb?s§¡w
‹?ït´š¦à?i®ÿº']?z,¢H]r'?\|ž/ð!?…聰°È?bH½×d?ï•Õù,c?y?ækú?XƒäKz™þ?GþO±Á±µ?‡z+mT?w†û¼äIY?ïmY	åÁ?ŽÄrÛö¨—?`ñÍ®è>ý?iÆ7Øl'Æ?6¥$™?‹AÝIT?ï1Ä/'µl?ƒ"F™Æ?jiùdû˜??cúÚQô­$?–z:ٚ»ƒ?£©‡2AÑ?îŽ0œwfá?†M'êYÏ?'eã†9Ð?zµZaj¿?›Ôψe€?}1·Y´VAGN4FGL J1405.3-0640?ì
ҟ}<@IàU!š"{À:ð¢nTqqÀ<…e®°'@qÛ$(~N@…ŽêéîF?ΠiA#?½ÆŠdó¹?ñ$lü'œþ@tP+çd~?áC"Lx?ïëقgÎÆ¿êÑ¥CñÇX¿ÇJ|ùzÖ¿æä_æo‹¿ïÿ'Q¦»ÁAGNbcuNVSS J140504-064056?ï–4·?yƒM…Añ?U‡BԎ֩?I¸k$?‡ËQmHn?xGDzª×?ï˜1ÿE_?{ó/söEç?VF|GjÍ?`=å摫?y"c¬ö?u£ 	Ä|­?ï\ÔkÉôù?€ã=ð{?j•à%ëß#?hqk)?'¶z ¼?{GwÎȟ?îï7Å-
?{d­
Ýý?ýò>iÕ?r,CEIí?"4{P¼?rJµaÊk?ïA"mR
[?ˆ4‰#ɖ‰?d}oè~WÂ?[´ÿÐ×Ë?•=ä[£œ?†ªt+w²Q?ï2Ï@xÑ?"þ–Y¯Z?p=lµƒ³?w'õ6Òß?•–¼¼Ö¬í?'6,Ãʞ?îìþ€£ÿN?Šy%Sù0Á?tÜÏû0²'?rÿ[9¢û?(ûôC
?†)Õ-¯?í'QÚp×â?•U7	ĉc?Ÿ‹k»8F?<¼$H?§%^"8þ¾?Œ+ìwG˜AGN4FGL J1406.1-2508¿ïÿ²Sézò@A[¾ãÕýÎÀ:Û»}0À<Vºlwø_@,¾yø¿?ÿ–Ù æ?¹'ßV?³RæVáŽ?ùˆ
%ð@
¤íÛ:MÚ¿ïÿ'¥4?ïÿÙiÍy¿ÚÜÜåHĕ¿ÜˆÖž椿æob¬c¿Ö§ayWAGNbll3FGL J1406.0-2508NVSS J140609-250808?ïàùp€ý?|à ]:ë$?D>*oy߇?H×Äi ~›?i÷ßÝӊ?|'ü8—A?ïÕôÓ_0?rY>¥w1\?Mq‡ØÐT"?TÀ‰;‹C?qWˆí˜(?lą"{N?ï uNò½ˆ?""¨¿HÍ?e9òh]y'?w"s¥N?™JÙÄ	¸?'³'
ø$Á?ï›|QyC?aѝIç¡?j¨,l(¦?I¼þÞû?'và'º¤ï?^ý)rÕ^'?ïÒ8߉W?uCŒŒŠÑK?Q­WÄf'¤?Q·nm{@"?r†"sE?s1B^?ï"7ïIhC?ˆö@–Z¸?Zy|ì+a?e]+[ÐĪ?‡¯"ü¨'í?…¨R—
T?î¥W´€?AÏ#o˜?hz+<á1/?uFïÛª?¤(ÙXÅk?œ'fÇì/—?ïê½Åë)?|ZŸp	³¡?}ÝGã&R?c³ƒzöLÂ?–+VOTíf?x|Ã}ù?AGN4FGL J1406.4-1654?åùg3*@E,ÔV.	ÿÀ:à翗Z$À<eôA…ÜM@v‰Á_[Z@_±@L?Ææb H¤?%U`?ìæ?ÇåTƒ™@퇂k?àM³¿ÞIMü¸!ð¿à+bùÌ	¿éD5囹¿ã»gêÊ䕿Ë58›ýÌõAGNbcuNVSS J140638-164954?"䫼?x'¸­œ¸?KøøÖMã?<£ÊÀsÑ?‡Ÿ?Ýs?wìf "øâ?ï¼ðwæ…I?uÑ»í¾œ?NÝ[ئ!(?R£u♋?}¬°N´'?sP•Cqm?ï\ýJTH=?~<còd:?déQTëƋ?`"Ÿ
?'Ã,…²˜?|Ú»ó
ç?"¿ƒþ?b ^å­?]࢚±¶?A¶Q]>ÕÓ?†"Fˆ¿?aâ%¥/=?ï=ä3""?y·sk©ê?[(ey¢ð?Oq"§X«?›…½-mW?3Æ«öh}?ïUDøcB?'i'¿¸!?[
ƒ´D?a~çA<À?"¦¤®›jq?´¿c"|;?î'Ù:]8?•ˆ‹ü¹S½?w¿ð¸ê¹?t»æH¢ö?¤nòû*?"›ÍI¡?îºÅa&>6?'špÍ©0Ý?sGŒWÐq?aâ"ßÉr[?¡ê¸hcW?cÇà\×AGN4FGL J1406.6-3934¿Þ± ‡<¨[@5z9'ÍÀ;2Êo${
À<œ!Äuæ@#14…×b?óòPµû?Ö|¦Ä¥`ø?ÜL³aì¯@ß덂4"@
^6¬j—¿ç‰Ò¡ÍðŽ¿ç/<B¦¿æ`ï. ¤»?Í#£×dÖ¿")xc,äԿϊ"=fèÂAGNbll1RXS J140630.3-393508?ïÒU,#ÁÉ?­Ò|2WJ?S"[³ö¸?g¼Ï	ƒ-'?rÈá€ò?ˆ(/ޏÎÝ?ïHýõ¹«?'L[é®Ý?c˜'£­L?uu›püE?‡Gœ
÷–M?ŠîÈãÿ?îón醅¯?":«µ?i-"?øjï?q¿/<e?žl~·~«?'ŝuʜ?ï2%ÍÖj?Aa}€)Í?@ž3",Q/?6è{¨õ?™6T§v©?mO©§?ïÎ¥…h½·?wýv,"ò?S9¿eLç?RC5óÈ©?sÞÍqŠ¡L?uj÷F}P?ï*cMNµ?¢]xõíÔñ?q=@ìœz?ˆµg¡°?šëcT§æÓ?ŸdûÉÛ?î,d6'À\?œ"	²'V2?kGüÍ	?rnhânT?«…<Úð´°?› ÊÛóë¦?í
 ¯vÌ?£³uòVÊ?ZA]Ua?]Î\GhDC?·*îx¨Œ?£Œª 0"AGN4FGL J1406.9+1643?ïÉ='@QjŸDÔEÀ:·í£ùoÀ<'"ͧ¾ @ ÔÇOŠVÜ?øÒó*öN?˅'òP¶?Ì£f÷ÛÄ6@³Þ¿=˜@³ã»¦´µ?ïÜÛ7ɚé¿â} _žû¿º¢>?¿Ðºèß'q¿ÛdóiÅ¿äF a3÷AGNbll3FGL J1406.6+1644RBS 1350?ï֜÷Çø'?e'™oã ?E+HÞҊu?3oÓ¿¢?rëÀº9?d"ß@&gœ?ïÓéV?z8g£ó"?P1fßÑ?T¡®ýh8?z*%Ìüö?wgÚ®Y"ž?ïPÜñ?†ðG?dhBò"â?dþ©Ž8M^?"WYuj¤ß?†kwÈ•Ñ?îõ$†êaÕ?wûµÊP|?sÛk4z/Å?VfOÎøÃ?œd"PÅÅf?v×8zP?ïºÇÛ»?r €¬£b¡?R†šŠ™šE?D4+ÿ¤?}úkˆ½'î?q˜HäB†?ïX%@´Ùš?'à‹(d9?`А¹'ªº?e¦O¬Ýæ?'áEÒ2—v?vÊæw?ÿd?'¾Lp4à ?oj:Ü7?kða€é>†?¢ä˜‹³‡?'X»p˜"?íH«ž ^?"Õ©Ùòi?'fì¢Bô?pÈæŽ>ò"?³s¶ÚŽ?"z^žy†AGN4FGL J1407.5-2706¿ì´I× ¡‡@@a輜$À;oŽXøÀ<¨¼ÆÅKÏ@!jÑF"@Hpa'ëO?¡6›óf¿º'ê?Nt'?ù"ÿü¥?ýôc>¾­?±f£M!›Ü¿î苤äPw¿×0ÄÃéÏ<¿×êäûAÕ7¿Õá!îgQH¿ÇÚÄ\:éAGNbllESO 140425-2655.2?ïú¸\A8?ƒWØ#Û?Vç»înˆ?Hb £""?Œ¤Z™§Ò?'F
þò?ï …c#2W?¿Î
ôÊ?z+¥êo¨å?‰O¨F?•djù?˜è…ÕÎ?ï¡c½i­?§®ûÔÇ?_õ¹ŽÓ?W5™CÐ;?œ›D/(
p?–Ê4֜:?î
·ÐrI?''¶ò'̹?pz‹[C?Á?\e#Š¢•?­5Š:%ø?'#@C^pñ?ï²3ˆ1?—?¼e?gåÞN?^ýV
›?œí³	‰?–QKè"åã?î
.%®?®Gšu…?ˆ?ø1Wû?—¦¦ˆÅß?©Xƒd|?§É§-†?îPÜW¦§?"¥}æPO¥?e[îÏì"?[dù^+?©¨ñºÃÂ?"UfÚl­?èƒË•ÙàJ?¯pé'¶?Ž%WÕm}?"3ÌÏ;½÷?Ì|*Ú?¯Ã¢5êAGN4FGL J1407.6-4301¿ï¬Ïô'7@1°§¨PÀ:Êõ\8À<B¾Ü-"@ߗ mˆÅ@Vç_ö	Ý?º‰ 'RTa?®`ÈAͪÃ?ò$ötfj@)¼=]ƒ"?ïÍ€°ên¿×.¡S!e¿ßÁf<J7¿á›·¡Aƒ®¿á'€ãÀ.Y¿ç*`Æê4½AGNbll3FGL J1407.7-4256SUMSS J140739-430231?ïð·Ò¥æ?WrøZÆ%c?:/G;zYC?TÍ?•?w?Y<¾\°?F½@®ïÐ?ïâÕå‡{?nƒ©bý_Ä?<£Ž=Êô?IDûBÄ?i–ziùNþ?jx5q€
À?ï¼ôE?Wâ?p†Â@õ›%?VÓî¬~ú5?bá\Ä®›?{ÐáÉ"3?jÌÅjSÃ
?ïÊüZw?X%)"QÍ?LˆšÓϽŠ?+ñ~&Äôþ?z©n6Ýw?W1D-œê^?ïê¥^ã?RQ¨z³?@Ú4ä÷åT?.z5á?a$ÀZ-]?P;bNó\?ï¥Ì€˜?"_f҇?P9'¯†
?`l6žp†?"…Ìþ¸çš?'Ä'"–ñ?ï•ò§k®?t3ihIô?_3˜?%?``ž
Ø!?†œã oo?q—úð
6?ïVæN(,?w*½©?bá3‰^ÖØ?H)	hžš?'ÇÄOB?v,AÞcühAGN4FGL J1408.9-0751?äAó9•o`@I%ñà'Œ7À8³çïhHÀ;Ls¿ë<ú@ÒèŦ¾@¦Ós¯û?¨g^«Sx?²ßß#;™^@	™>›A:@›¯|¿©Ý!-ÍË¿áFvÜÖ/L¿å¦@q	W˜¿å
ñú´g¿æºy
2ª¿ëyÍ¡^	 AGNfsrq3FGL J1408.8-0751PKS B1406-076?ïìWŽ~ªÍ?R"g''A¿?.qs'ÿÓ?¤F]ɜç?aÁZjê
Ÿ?Ql"ŒèîX?ïÝ7¶y=?k¦Ü"À<Ù?B×ï"à?Lê¤ &¦?n´ˆé?fæ&aQøE?ï¡\!H?}8 ß8?dv+,2ö¾?n-C}ØÆÊ?'‹n¬ZºT?x¡ÖɌ»º?ﻕzP(6?`·êŸ"?L{²•¨ÿ?1¥v%?~¥Ì±â¤D?_…Ð5/â?ïÓ»\Ð?f¾€7ٚ??9ߨt…
?0‡ˆ«'¨ƒ?t"'Ûbùâ?eÿ	׍y´?æßP?"7ORȬ±?VÜ^9ð?aŠ4(&í?†[ž=@í?'÷ÃŒŸ?ïmÙ[jMÀ?‹~<9úÊ?kØ#bŒ?uÃ:ŸÀÊ?" A¨?‡þƶ¸W?ïJ©ïµ?}ö^4?e…J¡?Q	W?¼·?"š.XDZ?|õ¤±ù€AGN4FGL J1410.1+0202¿ç¯nQ08@MO@Än&À9Ób ß9À<V/Ñ|_@ÖC€Þ6Ø@óò
s÷I?¶ôN›ï_I?· Täl|?ÿ‹…L»@
ùÇÚñS?׀ät^Í¿å)B™'¿ãï°A{ËR¿Þ{†^(P¿ìèné¦ٿïÿõ4ÊãAGNbllPKS 1407+022?ï̈́®·K?rÌՍíi?T˜q&æû?D
"­X"?tŒw"Ó'?q™·œoÿñ?ᆵQ‰,?a"®ýk=?[axé?mSÔxl?z/ùüg?tR?°h?ï…> ?…xȤÛ'j?w™|?€Aû»?'ÅfªÅ˜%?{ŋó8Pd?ï¥FÅ{
¬?aw_럌'?sô3à)?T1)h)‡?zD¨ùûXw?XÖXƒN$?ï¡tJq?wE0Ž{v?f´÷P&†™?V½úü}ò?õÀT¥?t܆Œ¢>?ïTb_?'ùL©Pò?gÄv½Mµ?s‡'Û5W'?''ÃͰޖ?Ž?qà%Ë?ïLÅ#Ý0?‰ÆkZc?øµ'\&ú?'âڎ®e?ŒÒ\ƒ¹ˆw?€ë÷k!-B?ïïïð?€Œ¹!ÏQš?‹0äٛÙ?ty'ÿ»q?'nvtl?u	«ÈXAGN4FGL J1410.3+1438¿í¿f‡@Pòy»­À˜À:aps/¢…À<[IŽ¿@Vp–ëêI@ߢ'g?Àe@ ¬s?¼ÂSL-U#?ýPÕ©²ì@`dÚEÀ?àý®(`q¿Ë¬Þð»¿^¿áƒþÿyó¿á¥?à?Æ?¿âlÁâ
&¿ç€[AGNbllNVSS J141028+143841?ïËñúï?a%2Ðõîà?UßøÝþ¡§?CéؕÇt?tÜ¿?]Åè­­¬?ïžo"k8?€ŸB¥<ø?bVk^UEa?gâKàæK¯?ƒÎ€HN«?yÖò<‹])?ï‰
tªd?wäißK?d±
ÔÖèÏ?j(Þpæ(ˆ?ˆ_YþÅ?rÛþ?îš]ª2̏?v­{âó)?Ç¾}Ñ'€?kºf!Ë?œÐkr&Ôy?rR!°‹ò?ï"y'.?tÙ÷ÁŽÉf?içHď?YÇèæΠ ?"E3í—?qÿ­ŽôÈ?ïa7¹ì?—U'(2I?rà~‹óR?w25ÀÔ?›;¹]'þ?"yZgˆ-?ï Fá³0;?'•Ð@²"4?p‰ZxnÁ?f'Â	,S
?—ÔÍ(:§^?€Œ"‹]wÈ?ì317Qó4?"]$[D˜b?£Å3Ê?‡,†êÂ
?´ƒí«²ú?£¤ó|AGN4FGL J1410.3+6058?ïå;Ӎ'¾@JÏäy'¼VÀ;ø|²F+À=* ë2¢@"o±UÍè?õf|¡;N‹?ÙS¸ä¸{Ý?˧À£ÉžD?ó0Ì5Î&@‡¦<•1«?ïþ—Ô¿ïö({ILz?éÙl€OF¿±R á·j¿Ò|ˆÛ—¿Á7»˜œïdAGNbllRX J1410.5+6100?ïŒÕë "?§Æ":N3?Iü9w÷²?h}')H?‹*Ø!½àŽ?¦ƒ$Ù?ïÉhڒÄ?}8—àT¾œ?J]Û²N?W
OÐtŒ?wÿ×:âȘ?yykO$p?ìªóހö­?¦$nkºÛ€?jrb†§‹_?v™Î™êÆ?¹ÔÍø=?¥Òi'›=m?ïÐÀTnlD?\à6~ôª?)©IǬ&?°^v؉?vҋ\¥×o?\qÐäFى?ïUp4Ӌ?œ©8P±üÅ?Kÿ9Äݎ`?[Ma,¡»Õ?"rÎQâ??›ëSá٘E?ïhµÄٟ?™_¨Nk²{?TºŠ5±9?dÅ{ø""?'± py>ú?˜pÍãb?ëŸ(àÛ?«¹3ZþÜÈ?nï""»Y›?{‡ÏÂøo?ÃQÅŽ¹?«ÿ=pŽ?ïv+"#vä?ml=` ¹?1#ïlf¯?/+á×q?õÿ·_ò?Dw1óAGN4FGL J1410.4+2820¿é[hd©‰@RÿCAžÀ:•ÝÞmAÀ<£xOYÚ@ï£ö¿ºk@
·Üz¿º?ÂpPJUl?»œzŸƒh€?øÂ^™éJ²@#JæX9?•"|¯‡¿Ôs£eË5ô¿ßéIDÂ|½¿Þ'G۶ʂ¿æ3OîTÜÑ¿ï´
ɇïAGNbll3FGL J1410.4+2821RX J1410.4+2821?ïÛeSÁÉ?]ÑâØG?]?Iÿ˜î±?8ƒY§>Zr?nÆ/oÉW?Zßêg¯»?ïËÏÒ1?v?³Júâû?P§*)µã'?Xùâ¶ÄO?uî¥yöŠç?rZH*xü?ï¦îþiÁ©?pŒ±PZæt?X³Y\ˆY:?J~/aõvÃ?ƒ-Õ,ðŽ?o
œµ.ªË?ïd3ŠŠÌ¼?hN^²u?zêX§ú™?W³&"N`?‰}ñՆi?cy¨Ão4M?ïÁM>ïvg?k²õB²6?V
@çw;?EŠç¬oªî?yÖÐ8iŒa?h`¼A¿¾?ïbñh—?Ý—(?`Ä "u•5?g'ü×$I?'‰K¾{m?ŒO²\ît?ïgׅ–
!?yìÖFÎê?eÅuOkWÒ?dŠâþ‹?L`ªé?vŒöc@6'?îl!
?"5Ö'sÊC?›w0zá?qfÀʧ*ì?¡WИ֝}?€•ÕÃ*1ŽAGN4FGL J1410.5+6215?ÛÚ"BB@J@8ÅCÀ;k
Çhß½À<»§œ'›ž@ŠK—Øú-@47yéÑ?Áe»È®¿º·¢™œ?ûz	Ì1œZ@´)Q.?ïÿƒVR¿çÞQ"'¿ãŒÝÞíᚿåÉ3 @|È¿ßÐÜH*¿Ò/ºÏÊ-AGNbcuTXS 1409+625?ïÁ¾Há¬?œÕ&øê?JKÇÙdâ
?GëÒ½;H"?|*§ð0Át?œÇ<¹ž?ïdꚛ«?'"Ï¢dûJ?skúkíÂ?~Kõ}ÄF®?CH2èK?‡ºW¨~&?îÎhM
}?'µ›¥.ð{?uEìqK}?w¸iQ'™? v—=Í)º?'QÿßÆ:?ï¦'{çN?ií­	X?gâø95v?W Rûp?€¹}k6îø?cþØëm'ž?ï¥0ðÛ?}5e†?a‹ª~ÕY?ZÿYŠ?'Pa¨Çß?€xSžF?îo•Ô?§ÙùÎ; ?'ü*Ç¢–?Š´rž×?¤Ç§"œ?£êu"Zzò?îi§Ê›?˜µª"´IÁ?ƒ'EŸŠŠ?HíEï?ªß"Ûg'?–Ê}½'I?îƒØxì>Ç?¢aù¡ƒ?‰4©ýUZï?5I~¤Ð?¡uMñ
ÕØ?ˆù*"ÖŒAGN4FGL J1411.5-0723¿à'À긽@I3ÞÑ·À:ŸÆh.½ƒÀ<]ùú,h@ ó¿ÕÃk@0«Ü'<®?Á¶f2¿©b_¤3@?æùžßY—?÷Z®Fú»H?ä¥+"˜†I¿§Ež€ð;£¿åø}àU•´¿Ý3žÞ'>¿æ"1l"Ž?"bèyóÙNAGNbll3FGL J1411.4-0724NVSS J141133-072252?ï
ÊÉ3Ýu?™…ÃœúŸ?_æ³?Râ/°b?œ¶†¢6šH?™(œ›'ë?îþe|Kü?–<7Ãژ?‡â¡›&Õ?'¯4*v?—o_.DÔ?ÆbÞ:?ïZÊ%þ?‹eZ]Yý?r	S_©Uö?pe§Ä"?˜:_д³²?‰~)W€?ì°5!Ó?Žx¶õõåö? ‰:Mo#Ã?}Ÿí:¿eN?²9ºAŠ?‹TŠ×ðþl?îf NzȄ? IZëG±ü?oX—"ÞSE?c?¥[hŒT?§ q›•öŒ?ŸÈÏ.Xö?í/]&\ò0?°Ä˜Ùo?•8Ä.¹H?™ ÜI™?±6åÊ֚¯?«'¯˜ð'?î(Ú,]´?™–—ëö\?'Èiӏ©?€5a¦ƒü?¨À[š‰X?—¹"Š?æ栀ò~?£`5-8'?µ±.Vl­¯?šÛí¬†?ɌæÒKU®?£È&1Þm‹AGN4FGL J1411.8+5249¿æ§ù ñDÚ@N!uŽ!–SÀ:ÎÜيJqÀ<ÐÒE²'¸@mòGۋ×@'åp1Á?¹ù⯍ 応Oò†qã?â¸îÞðeÙ@
©3)ƒ?ïZTª|?ì¿ä¢ŸÒ˜¾¨¿ÞíC÷Ò¿è~bÁ–7å¿Ì¸éÖrèÖ¿Úa€Îq"AGNbll3FGL J1412.0+5249SBS 1410+530?ïÜ/¹+/Y?"TÚúlU?7>Uiˆsx?0r ;G¹Ì?pt>&›T?"b"ùR?ïà.BLo‰?j8\­GþÊ?8¤¶¹Ä…?DôQÓÐ8?l¹hâܟy?gcÏέú?ïî¡w£>?¤	O3?Tqaj´Å?VÀňL?‰65'ÊQÏ?:=÷†¯?ïçBƒÕ"y?H‡œÀFéo?<½hƒñ$?%d¯Se?e%ÏJë©?HFã%,b?ïÒá–ÞS]?tÓ͟?OIFýEo@?KÔpb³¿?r¦Ëä­?rž»ÉBŸO?ï–s©'W}?ˆ(5Ô"V—?OsmšY)?XÕc­¥l?ˆkÞ»Ûº†?†àm›zJ?ï"8™Ïtr?Œ¿þ=<"?`ÞWüýªX?`Šq-ÍÂ8?™!¾Š¢'?ŒBRÙîRÁ?ïªO3ïÆ¢?k¯eÆFãw?WQ"€2=^?Iª¯ÛܗÜ?''­€Íä?kxɼ3dAGN4FGL J1412.0+3836¿ïù,F7¥@Qg¸d"À;†2´ˆ2À<Ž#â]@ ˆÂ%ÔÐÒ?û´{'G–?ÉgöHòL?½ËPËÊnN?öÄçûý<@ì$+#¿ïÿìêy…þ?ïùàÌ^¿Ö ³Ô®C¿Úf÷~0ˆ¿×>?©c;¿èr'~túÿAGNbcuFIRST J141208.2+383521?íâÀk·Öh?ÉA9ðš:?QRL,I?t}¼—î?°¤³p˾1?ÉŸ~J?ïà‹?ƒ?p€sá®Æ?@B"Ũâ?JµQìÒzj?kdU(G?kÔ2'õ?îkV96qE? «N‹žò.?d‰0yE?h?vì+Ä`—?¨	cŽÂ;? <HÖLl?ï±¹Y2w?_Cþr7[0?Yœê‹#??	káуŠ?€^s(ˆ4?]kUüpZY?îIÓÚ;?·Ð¾`,Î[?[ƒf]t?s<–(¶Û†?ª†´ÿ¹ä?·¤ÖFp?ï™\ÁT§?†ˆeµ-·?Q(7%~Õ?Y¶'Ÿ‹WÙ?‡•aìþZ?…rÈ÷	Ÿ?헪 ‹?¥eàx×?gÍÌ¡¿«?vZ^¹%}v?²"Aw&y¨?¤å—O
«à?ï:eg°5?{bBd.v?gð¶´yA?U4sGêá?•±¼uó"e?yׇC‰JJAGN4FGL J1412.1+7427¿íj['Ôþl@DÆ	VÀÖõÀ:¢!óoÏÀ<£èì¾Ü@}s±¨"@‰Ÿ
vá?ºüg>ÀZ?˜Ð—e?}w?Þx~a.ï@­{£ºZ?ÚÙéëÁ"š¿ç E…EO¿âªÜí¬@e¿àyÊÇ9¿èŸú¦ú«,¿Øx' Ï-zAGNbllGB6 J1411+7424?ïÕµj@̵?eJåIú‹?[³H©Öj?PçDöë¶r?l¿¼Ey‡…?_Æ
Hé'?ïÃØìã&?sñècvßë?PAu'ÚÝ?S/D˜Á?zy!""??qe…ÈXØ4?šÌ?€9u番g?_gd`MWØ?` ¬tVf?‰+°ïz?~–^½~?ïi1qçú?déÉþSg?näW¬/
"?K™¥Úí¤?",Ä(ê×?c‰;T¡6V?ï§
ï$ï?z§¸PËíÒ?lñÕ}E'?c:æÚaÚ>?~¨¶±Ç?t k÷ž'`?ï^ɐ˜o?‹>²¬àÕ5?]wÂëí?dfÞ©Á¡?'OQäޘP?‰˜¸'Œ&Ž?ïìX"}?þTMAù¶?n?Zù•Á"?oÞӏÒx?™–—Ç+7?Š"BWXûq?½DĀ?"ÚQ=áí-?‰]ì':P‹?ld‹by½Ë? L‰"¿Ö?ƒyh1O€AGN4FGL J1412.9+5018?îŒ}~}Uä@OHƒýP"À:õênžCMÀ<²Àsøö!@ê²:O\4@SÌÐþŠµ?蛢Íu¿]Ô³tV×?˜¥w¦Þ.R@	J«GA1¿¦À"üêæ¿èh'Zà÷&¿åBl"4X¿è…y¼"€-¿éKV?§¶¿ïÿ[•R<AGNbcuSDSS J141302.28+501927.4?ïòw¶ðÂu?ØD•RW|?=ë±Ç· ?WYÐr=?S•¦5*y'?zŽVa
?ïÝQ^]§?rˆZ?±,É?AÖ:SÞj?Läx‡OmÅ?n9_ÁÑ-?pUñ<¯?ï€oØfD>?…‹÷æ1×?Y}ü¶?/?^)ðõ#u?Œ´JjŸj›?…"ŽË4qL?ïëiñò\e?CR]]iã?LÛŊ¤Ž?30+Œb$?Zë.{Ú</?=ýO<ô‹O?ïá>VQñ9?pF°N?MÙ¤Íðó?KÂ÷¥Š
Ë?gK@j³8
?m3•™²Ö›?ïvݮك?"Î1á*{?R™YÝ°
?[r0/m?õŠ ÎÙL?"\CκL?îýê"vO?'T`ãPª?ch;VÛíq?^ž¦Ô$?ïE©c?''¡0qí?ïÁ£[ÂÒ?c3"I2?dy|È{[?S	ÂWC)ì?táïê£=X?^Áù¶AGN4FGL J1413.1-6519¿îu=HØÀiØá®aÀ9»1'À8jÀ;'™,ŒP@ۓÜ@]=@ý"$½N«?¼2sÓÝ?™æÇþ9‰í?à.ßFL¬@V†PÀb¿îæÉbµþ?ï"2¼ë®9¿ãbà՘Mi¿á™óÇ™k¿æ)'@¶©¿â"¬Ø:¿AGNsey3FGL J1413.2-6518Circinus galaxy?éä}/M?²Áöµøv©?l.»»Ã?^Û»u2^?Çþ‡ì,?²Ÿö\S˜"?ëçÁè¿?ºµ—&!Ò¹?_=½—þùk?eÊM3îþ©?ÃQå}J1?ºfrû ï?ꓝ¨`ˌ?©î€p§Q?ŽÍ½y¿9?"'.L?ÃÄ­Œž<?¨LÞ¤w	?ìÕ8Þ;×?ŽÂ	¡Õ­e?…嵁²õ?d oÆW*?¶™ˆÐCç?Œ˜
­†™3?ã,‹lÉò?À=,ú<¥*?‡ZùÐÚÜ,?yÿ6[ý›è?Øì
ˆ»?ÀNøۅ?ã‡èŽ^0?ÈÃì‹Px
?m?ÃUšÞ?€†Åb'tÌ?ص¯Äÿ#?ȟEâÚ¢›?áyy.Ñ{?¸"§ ~¡W?¡ˆƒ?,i?'@`B_öá?ÚÛùóBúž?·ÍÞë]…?证¼}G?£W¦ÓÂ?›i£eS?€ûÃcü+›?É߃~ú?¢ÛñÎ|AGN4FGL J1415.5+4830¿ïÑDô¯G‰@O~Ü~ñxÀ9¦tÿ†À<K'5!Iý@Á½CÚu?þDv×ͱÏ?¯z4ú]©©?©ÎЁ6ï?ú#ÝTÚLè@Âƒó•¿åMðMÛU¿à"œÚ–¹ë¿Ýý±¼P'á¿Ýš¿]οà™xa"·¿Þòky˞AGNbll3FGL J1415.2+4832RX J1415.5+4830?ïúU«¥'(?0Ø&ck?
úþè¶?	¹dd?CòÈl0œ?-ã|;.f?ïäÀ?[ñª?htq7??7̗URƟ?C0sÜ^?hF-×ü©?e©‰uò?ïÀ¼"'¸?qmAÙ⇑?O» Dž‹‹?8éwGå?{ªŠæJÄ?q$Ž?ïõåwh—?5ýY6'-v?!;p=Q?Û­ôÓm?SÊÔ
)§x?5caÞigþ?ïøëØv?;'J乑ç?$"+€G$?ÒX­Žù'?GOkd°Ó?8¹0´Z?ï©è´"Ì?ƒtÒìȪ?JÇb쒝?Uí¢ôûÙÄ?"™jZøÛ?'"ÐfþŸ?ï'}ÝÀ(é?~CLœúA?[ÚpŠ"?`!ƒð$i¼?ˆ5Îßo¾^?|ÜÙ«F±?ïâ˜Ӆ_?XS¸žøj?5xú;b?"—‡k1ù?j¶
O´õ?W6ø3èAGN4FGL J1415.9-1002¿°9©üG¡›@GǤô^À;Ep÷¹àaÀ<Ù¤?åÉ@ÿ0,#@SPÊï?׿-BÖ¿?ïÿþBe«+@"ÚųÔ@¿?Æi†¿ãÍÍlê?Ѻ(»
,ª¿æÁ|^¿ïþaßîé?Üè=)T¿ï^-ôAGNfsrq3FGL J1415.0-1001PKS B1412-096?ï¡Bµ(¸¨?"†î, -?5Zpÿ?"L hK?içáJ
7r?jµ×à®ß?î7#y Ð?µj™jA?š"µͶL?®¥ïfg¯?ž†ÛÎ]ˬ? ‰¢µßæÔ?ì•MìÝJ?¥ûuÖÁ¤B?®aÀóÒT‰?¢¬ª¾;,?¨Im½_ÖÜ?™àÉ
b"©?ï.A"À‰?ŒÅÒB?†?‰r%à™›?†ÁýÙµÁ?Šý"ôKõU?y¯3CU=•?ï&ß'ƒí?£<»žÜa†?•º}>ïÿØ?¡¢ƒk7?u¦…[Mî?zEÔëÀ?êD3øX¤?ÆÖ$dcVç?¶Ç‡§·f?ÀG>sêC¼?·ؖ{úD?¶îÇsq'?ë#Xìøˆµ?©=¡€K?³QÔà–o?¤š38	Þ?³"d"ñé?Ÿ(fóÌbf?뒍uÁD¦?·ü'h܀?³ÌSBVÄ?µ)U–µd?°gÇÿý^?¢7ñ80AGN4FGL J1416.1+1320¿ä±ó²ê£w@PyÛ
Ø0À9ÈÔ¨c`øÀ<X¼ˆ±êÉ@*ËâA(>@*ÈE~R?·h_ºÐ í?Áq}ÝÑØ@¹Ç¼Â"Ž@
{NÀWs"?îB # –x¿ãñãr*¿Ç¿äQ…¦ž¿çÕj*@Ej¿ã×MŸ7¿ðAGNbcu3FGL J1416.0+1325PKS B1413+135?ïî'Båi?Qâ°ìøãj?@àìüî`?7gݤv'µ?[Ar•6œ?L±D)ï»É?ïÈ´ˆÍt?u'eëué?Rƒç#7Ú?ZÒU³ŸÙì?wÁݼÓj?põS	ÚwÅ?ï»üÓÙ9?lP•ð‹Â?X%O™hë?TÕ±LG
?{øB,³;?jgT­c?ï'Õ"¾àÈ?c–©5{?w0õP""×?XL
ÒçM?d@?Œè?\]°N*Ê?ïÚ&§‰œK?býáz(o?W®;œÎ?Q%
˜Ƶ?jQNv
–W?]¹;ªhP?ï_ÉSÆ{¥?fWÌÅ°?eT–Ž<?peƦ¤?'\B¼Œ9"?‹Yd§ڙ?ï'évј?|œcâIT?fél3u†?fÊÔ ?‰‹GUÛÒð?x®o'W}?îč3b`¦?ƒ"¡L	Ӝ?r^·Þb¨?wÞ-Dù.?–ûúÚº?{E´ÿIvjAGN4FGL J1416.1-2417?ï\R6ÆY@ATïܜM©À:—#	¼AÀ<e¤m í@ ÑD€bï?ûI
Öק?ÃpÁÂ؂?Ãî•ç2@&º «q@
	œºá<ñ?çžX°›=ß¿ïýf],+?ïæ¥á{…‡¿Ô¯–[ ¸¿á·¾þX
-¿áåàš	+AGNbll3FGL J1416.1-2417NVSS J141612-241812?ëöˆ¹®?ЗÙ®‡'?£e"ëp?Á=ÁªbrD?¶½xÜÍ°S?ÉZ™øþÈ·?ïÓ[gð%?u'£Üʎ?K[ý6¹î?U "sYvc?ræÌރ™(?qüË·‹†?Xksc?^8•T?`ûä<È6?r}3ƒLg˜?¤eÚZ—	Î?`'b£Â?ïQŸ';Ùö?u•~°I?]	Œo´HÀ?M*°.¤Ð?"ûvñ]º?tÜ,oÙZ?íØ|bÆ?¼Y
Pn‹?"Ò&Øû¼÷?ª1℧Á'?¨&r1U ?³@& ¾ ?ï~ºdâ¥?Œ¡Hâw?_P'ʉ"Û?m61ë4–á?ŒgTrÔûô?ˆ¥A(Ðiö?ípïþøey?¨Išxó¤?a[ºb%\Û?n£®Iï­5?³í¢4'ºÐ?§ÿ¦'¤ú:?îZÃgj¿´?' 쉫æ?oTt}«©s?k9b>'õ±?¨^'C©?'‰•ecyPAGN4FGL J1417.9+4613?Úàï-†÷@P§Ú¤ü¤À:ö¤}"jŽÀ<£QùÇכ@^"JÊÿm@ç#? )?ÆhŠ'¾Ú¿ž"$\"7/?є¨½õo@¬Y=ÞÝÆ?ï¿á—_,¶¿å¶XKñp¿ëÐ÷Ÿnd¿ëñõáõS¿ïìu߀-¸¿ïè(‰ŒAGNfsrq4C +46.29?ïÝs¨e±­?˜¢š‰¸·?I dç[N?jbŸiŠ±?lD>Ò-sÓ?˜XŽØ«f?ïÆo®—5D?~-Ém]?T'òV;›?cù*­	"T?w£l!­w?v®Oâ(8?ïoÿAi+é?ˆåÂW¡ÿ#?eblK¢©¯?nã0*üá?Ž§"‰-s}?‡ãò'|?ïڎ©¦'
?UûDÏQ?c'¯¡õ?Pn«Ù1?aߦ…›£ö?Eçh+Òߓ?ïé_¥µL?mrÕåA99?Si"Kߗú?P$¹ÿwz?Y×!¼t¯9?j´<LªZ4?ïNk,€?š
Ǽ}Û?e¤/ŸRß­?wY'ãŞò?"~¾ö}ÿ?—:YOùþ¹?îøϱÐê`?'‹@7Ò?tš´;?{yhãsv?›¿‰Zk¸3?Ž¼RÀ½?ï$‹X@ç?zrŸ";ƒ?€óu;?
?u¥ýô™?}†ÏÜŽB?gH¡Þ'
AGN4FGL J1417.9+2543¿äÖUÜ_¼@Q¦W>«6zÀ:l–ç7²À<N1©Æ7‡@"Ô˄£=\?õ˜¡Ú°»?Àh3›
-?½âËfÆ2ª@9f1A@Ä3D{-¿î3ᱶF¿ïµ>ì¤Ù?ïÿë""i·¿Éçã(®ÊÙ¿Ár$	ʄ¿» !6ö%AGNbll3FGL J1417.8+25401E 1415.6+2557?ïGc¨W3?®ÇýOä~?SÙ¤²Š€?Eß#ÖĆ+?•áÂJ?_­±öÕ?ï‡òDM`?'ì\ɪdŠ?bŏ¾'Ý ?l*·Â"3~?‰R
ïJ·?'è/1y}?í}¦©
à?¢wng	ü
?aWøóûy?bß"o(Q?³ˆ
ïgïb?¢d&¥n)¢?ì{(w9êª?˜¢Ü{7?p»°"¿…M?`Š*.àdÆ?»<"Ú_?˜O×Qåq?îôLZCë?sGwK'?bñÜÚ>­î?`gÌCÅ9¡?Ÿ9zeê?œOslb?uÞ?§yÔ(÷ö?t
{É+u?…¦nîã?¢L䦆‡±?¥MêK¼À?ëôÚV'öÒ?§Fà·³A?iËôEó»_?m|TKF#u?¿ŠÍ¬yMÒ?§Ž'Ât`?çdcLÎ?°ÞY[Úr?€/æ‹.ƒ¶?zнÞτ?ж_°ó0?°É	õnàAGN4FGL J1418.4-0233¿åã­C£@JÓÙý6÷äÀ8>Ùtzü À;Q‹Ï¬{@Ë¿º?ú<¯c/zA?¤Ê"0'o?´€$þg#¦@Äpë$¦¨@ÓAaRü?ç¾¹ä"¿Ý=ëì:¿×_nû`^¿Ðqal+¢E¿ßÀÒÆӿáO	ß3ØAGNbll3FGL J1418.4-0233NVSS J141826-023336?ïñÁjæJD?OF{ªµ‰Ô?BõAú—Ü@?=göW?SˆÉÒAb?EÉ©.h½Œ?ïº
.ú`Ñ?w¤áŽ·P¬?VÏ[p¾U?_ŒbD®j?}G''&t?t;i®‰‡?ï:Æ-)?‡Ïâ£E6b?mZÛªú*?{_çý?"é,àÐé&?ƒ¥Ã~†w
?î¾òR(§û?†Ÿi_âÕ?mœ´'†^?Q?%8*Š3?¢@¡/ç?†íEq÷?ïï‹Ï½©*?Q9ѳÎä?:2S^ÅO?2gNÂA@?Z[ÌjvN?NHL-N?ï8à¨+Õ?˜1ŌöúÇ?j¸À*›í®?yuéÂû‹?•ŒÓ^
®?•œè¼>¦?ï|ìûžúà?åšòá¿?nd"¼0?{ŒJÕ?‰+¸^Ž}G?Šð
×t"©?ízk¡Â:«?Ÿw 9_¶ä?z$$÷Ô¾?d¥_"ª•?²Š`°]Å?Ÿ•xym½
AGN4FGL J1418.4+3543?í¶ö )@QfY_í¦aÀ8'cxu\£À;À®ã­¹â@á¨0¶+@ Á['—?Ÿ¸ådHT?°ídášÓð@ÙÂ~•1@fTȯ1?Ô"g^¿àEí οâøòÔô¹¿àŸ¼ÞÃp¿ã¿''Œ6¿é¨¸á2ŠlAGNBCU3FGL J1418.5+354387GB 141615.9+355650?ïôWœ¸Ìª?H¾úàŠa?:)€¡©?,ïg
'?PƁçÐù?EFe|k4ž?ïÙ8|·ûH?q–©UsÜ?Dtsû)æÏ?Ov?¦E=?pÕ3"j+Ï?n;Áç1x+?ï»üs¿¦…?z†0–¦'?a»pMTÐr?p`Ãؾã?y$
Ü¥Š?t¬RðÇ	¶?ïüòVÊ1?"+%¢ü?	Y\s´ˆ‹>ù"‡<R?5Bïí€Ò? Î&anâ?ïêÕêéԁ?g˼^?8Ò­¾¦•N?0«Ó§¦ Í?b¿nHÂ?g-q¥!H¸?µ°?ˆFí¶bŽQ?W

d*ñ?jñPŽ²¯?‡ý¬=²©?†	ëªø*?ï 5‡ï?…q‹¶ìŒ?`Ë;¹Íí?lÊs{¬¯…?ƒ­u4ݜÇ?€&KÕ1?ïù`ò'µþ?<a'ëÅx¢? ÿ¶L?äzönUÀ?G8v5Ðr?:ëâ–Åè'AGN4FGL J1418.7-3504¿Ûwô®=?§@8xW£UÀ9õ\ŠD'À<+!xö‹ã@qªqX1ð@.…Nˆú?Ã;™‰(ˆ4?Ëz$‰LD@Iæ?@0kؖ/?ãaýKÙÆ¿æšáBO°Â¿ê]3ímVE¿êšn«¯EÓ¿ï VíLŸ¿ï÷6ÍòfºAGNfsrqPKS 1415-349?ï¹âõê9?u:<–·?kÐB¤Ê?cÎg%Ûá-?u‰mN"|÷?m·ˆVIŒ?ï¾±="?žeQ—1_?‡ÉAͶÉÚ?®µ 
®?"ƒˆùèÂ?z28Eó~?ï\ŠÜ"¼?…ºÆ›ør?zšµĊ?{W3‰j…"?‹«ÂÁ$/Ý?~zKÓ®?îÎãŒpªý?yÜ¥©è‡A?'ˆ‡—qG×?qG¼Uiò?"›áX‰?lÄ¥pnÜ?ï^}Q˜Æ?Ž;›q?€ìlÏ?|"@6wp…?‡t(nŸu?…K¶TÍ?íj=ŠDp?±¼ß?9R'?`¦Í£{4?¤ûA….?ª«Û"ù—g?¤ÌJÉo#?îc VÐC?˜"ß'É?"ÆP\Pó?JÞ°t|?žØnóQ¬?{rc¶
?ì–å¶Âc+?– òñ}?«ë÷ã»w?DÊGQò=?«}¸—ªŽÜ?Šå—ôÓÒAGN4FGL J1418.9+7731¿æ˜ŠL8–@CI›Oe™À:^§Å¬GÀ<u¹&&Û6@ fhê¥%?÷ªˆºNE?½ÊèF$ý?Én#Ê	£î@aNÏq@Ñãá'Tý?î!ƒ†Üþ¿Ô?Íà?dÅù1§¿Ì%œq».¿à:aÙ¿àÅþ¢ûrAGNbll3FGL J1418.9+77311RXS J141901.8+773229?¦—Œ'?oÚ
"?€D\#?vڜ"2¼¯?vå#î5?	?o´ß	+ ?ï­}¦ÞO?Û*~Û™?a‹"ì‰G;?hùÇ_<Ð?€=±1ð¡?z[Ž%g,?î󝜲ý?'šŒ
	?‰^‡IfÐ?‰àWhþŽi?"ÜýÂD$ö?ŠŠ8áD"_?îs.$Íâ?€®o󺘴?*ÜÎ
q?`)V¬Å%?¤çÉ÷\!Ò?~~º;x?ï;zæŒM?–Þ¬»bÖµ?'F³¢íï?]EPM<¢?‡£º°ÂÛ?ƒ¬÷Y½/|?î÷][È5? #´lÝ±?xÙ½Ñç$?†é›ÈD"?šÞߕˆ?šÚ^ÓÕV?îp€Ây?Ÿßåölíå?œëNä¸n?–`¹'ë?¡cPü)®;?"#¢—Ÿ/?ìSÇ礃F?šÒW9ówÏ?|ÁáP+U?xã°¬L?¹²(†±àb?š€š9	8AGN4FGL J1419.3+0444¿Öa|$qW@M«=ÈK^À:¹Ïþ°t§À<†ËÈ1]@ ‹ÆGLš¸?ûÑÁ(SÜ?Ñi‹ T?Âxš$W"?ôÈoU"qD?öh\૦â¿ïû9\B 6?ûª0¿ãA؉B	¿×­eL`¿²lTg
{.¿ïü-þ@`AGNbll3FGL J1419.5+04492MASS J14192748+0445138?ïFÄÚ¸Ñ?Wсêâ?mþ¦¦Tãf?™½ÃÌF_Î?"gª‰+s?‹è­†"ï?ï¢ùlñx†?'xw
҄°?a3ë\â\?j²ÌÚ²hF?'ÿ×͚Í?|Wrù‹ãt?îú=ƒ÷¤o?Œ#Åoð?sèº õ.p?t_Rª(©^?›¾ ÷Xy?‰ƒÇæ­h?î21—…?…=g¥óÈ?"õzÀæd£?q™Ç¼jŽ?§¢/Žd¼€?'ÊǍ•xÑ?îÂÉ&,Ã
?™?6\Û?m6'ÿå?p×cñÅiQ?¢åý¥|?˜
KGE»?îùEs§—‰?žfšWžfL?q¹m\ÂSB?gÉq½?œhö,¥L?š±u¢QJ·?íß8è(ó¿?œ¡l'Ò[A?"_zž]¡ç?†<åéJÑ?¬ô'Òi¿˜?˜·éƒ4]?ëóƒÈvü·?Ÿ®j6)²¬?‡±EÍ¡?"KGš¿?¼AõvlÌe?Þ{°VrÉAGN4FGL J1419.4-0838¿é_Þ§73j@H-¬îàóËÀ8o‰u_'®À;§™Ûøó@7ë@Iݙ£«?¢XšËÈÀÏ?´':,v«ƒ@?-É@ÒûO—¿ÑµPx…x¿áOY"J¿â¥j­¥j¿äš÷g«
¿æק¼r¶¿ë‡4<G®ëAGNfsrq3FGL J1419.5-0836NVSS J141922-083830?ïï˜
Žš?Q7ÌÆ|܌?:Ù!ªyýÉ?0{Ê?[‡îCè?OÁx®Â¦?ïÒ\#…~?pV)Çjˆm?E[&áä›6?MÇíÊS…
?t&‰·Xà?m'‹	d×?ᄀœ?v]¸1•?^¤q_ ög?hîs×»X?yIߨáÿ?q9.îטì?ïï*@‹—?CñÍ+•"?2œag)?·…Q]?]g¿½s?B_u?Çô?ïÛÝâ°B?f«Ñ;.È??€µ÷—ß4?7*1@O¬?ppMŸ·í?e!.Úy)Ø?ïy-ü³Ý?Žülé"I?Xê(GZÔ*?eÌÎ&Ítì?Ž—;òÿ¤V?IÕ˞Û?ïžXø>Á?C˜:¢?dd9ë}á?nV¦&†+È?ƒb=r 4?{wcr˜ßB?ï،ø—è?b-ç܀?E)eieC,?695[Õ4?qÍP!§?`زِkAGN4FGL J1419.5+3821?çÇï
—ç@QfÙ×À9×À¥wnÀ<=®ä"yw@ùÁ3£'@"ª¼×ŒC?·‰êá¦?ªA… ,I¤?ð\Kv @
ÓìÆè1W?ê<C²\´¿Üœ?¼-˜?¿çßáa¯G¿çç×_w߶¿ç9ö X:)¿âzŠ&_AGNfsrq3FGL J1419.8+3819B3 1417+385?ïõ,1-ÁÒ?BœÑ
eêì?3Š4ì#?!IJ+¨ƒ?Pã<Ñȯ9?@JJéÙ?ïÕ^üº¦/?s#ð¶m±?Gqþ[€-9?Rcÿ½…?rbAå¼ÖŠ?p‡,C§·ü?ï­þœcߊ?ulX†:u?^,Ð9´Ì?b–™Õî¥`?€º¾Û²Ã?r­võB X?ï¿ÖBò?ZíÆÉPâ?lF¼›?OTQÉä8?r»v®‰?SÕµÃÅ?ïíS§¿Cš?OÄ«þ²®z?AIÓÁßÙ?0ê$#¢?\³Æèóy(?Lv_\	?æz?Y?ŠrelD?WLIÄ­	?bÃ3¦â‹³?ŠóDä>6$?‡ý£¨gòë?ïoCó•ö?'r㘲f4?i{Sâ# ?pv£ŒÂߤ?ÐwnyïÖ?}éø/ê¼ì?ï:J?zé,¸õq]?†[­¬ŸP€?pˆáÕæX'?‹ò'¡¬ú?r®/xG 7AGN4FGL J1419.6-5153¿æmÚµ(ý@!Iz»ˆÀ9W"Iô?ØÀ;¨e­ÙÂ@	$ÕøD @§£Àd¾?·<TÄþLL?´4ƒjX8{?öƨü
,8?ô¢=õƒû"?ÉZB×%+¿âŒ*°­²U¿æ;Þ}yR¿æ~T>p©
¿ç,åÁX¨¿ðAGNbcu3FGL J1419.1-5156PMN J1419-5155?ê¸@MÍé?Át-h1Ü?}}Î3='Ý?uZ(ЎºL?Ƶ0Žh8#?ÁZƒ×îòo?ÝtášJ¼?È&†îWr>?ÃeE¿|Ø?º`|º™L?ØØ{…÷8?ŁùÕC"Ô?èàE]?°˜³—Pý?¢Æ¬&ƒS?•gŸx5-Ð?ËÒ´mZv?®'ŒÄzìü?äwƒý{u?¥MERÐ?¿ËâÃJ?—eäDêi?Î<m²(‡? mœ$^::?ä½pv¾*ü?ÂG¹˜ùœË?bñÝjŽE?†CÛE7L?Õ~ïõô£?Â$="ÏÊ?ÊéU
ùgà?Ä×àQ9«?ɐ)ÐwÁ?ö¸EM´`?âá£2
ˆ?È͌üÖ?äPH+V´±?² ]3ø_?¬9Ö\å×?—CZÆë¤c?ÓÝhn†ùâ?±â$ÐÁdi?×·Ü2Îçã?«³¼Kôjä?Í»f»ÿRº?§LÉ@Ø
¹?Ùjpo1nÁ?¬uMmÇMIXED4FGL J1419.8+5423¿ã¦Ë[ç!@M&É[ÿWÀ8íL§xnÀ<MäHêT@v"Ž¾@¿–Aö?¢K†¢W>'? –:iˆYÖ?ù×Ì%Ýà@F˜T _¿µ
[b ¿ãÔ ©Óy¿å4°
õ'¿äØuâÛ,¿è!gßjr¿å¿eÁ$øÞAGNbll3FGL J1419.9+5425OQ 530?ïíiˆbm;?….¶S•?7chɖhÊ?cTxoØËù?_T3¡uº?€a¥ž?ïÐê!Ä?rì=z9Ð?D³ðÎ#"3?NŽ¢S±?tôsVz:M?q`#åæ	?rnúV?rl}ûùI?Sßóè˜?ZÕ·95(r?|Eà³)O¿?qO¾úFã?ïúM#³J?/‹°@æ‰?2¬/†2?Œ×‹
c?:ênw?'hÞÔ±?ïçø«?\nq|3ø?4‹àd¯¬?&»È.Z?evƒ½(ÝÌ?["ŸÞþå»?ïw¾W`†u?'Í	2®¨õ?VÝíŸíÔ?ftûրÏÑ?Oîf
Ý?'Eâ&?¼?ï‹iãs'Y?'ÆVfÃ?Z«¸‹ed	?WX` œ?‰ÐLCd?€þC"÷8?ïñ=2'ù?N–g×?I˜I"ØÛ?<…ìôôó?P¹²¤9©?D=»ÉNÉ AGN4FGL J1420.3+0612?íÉÛ<•÷<@N!	á*QãÀ:š¢Ûa»À<^{Ñ1¶[@9÷8Ü"@®"ø?¼'¡Æ3+¿²Ê'+'u?õ7u'c/@ñ.ÖØ?ïô˜ú7¿à×Nó[¿ëâËf›@¿Þ[*4ï ¿ã«ØáX&¿Ýº¹9r•AGNbllSDSS J142013.69+061428.6?ï߯F:]/?gæýsû$?Ic2&O	?AÏÂ}¡Ê?i÷í]Î(Î?eN;k Àà?ïÕEr·â?rtm/™M×?FUˆ"EV™?S¢-vÕE?r'•"ÚxÁ?nN‰¥?ïd‰f	Ž
?ˆ2@EÊ¢l?_ó•'éœ$?aþƒU…?'o™è_T˜?‡Æw}Ê?ïÊožãb?X…æ¨ýÏù?_: …áß?Fáœÿš†?rùˆph$,?SB,;šz]?ïÊ°§Ê:?z\qD?e?W‹œ™9à"?R¹©Û	iI?tÄÄåR¢¶?w²yt–?ï'%®»??ˆW&'h?VtWŠkã?`;§f+›?Œ°+®¾?†Wç{,y¹?îþ•zâ/œ?'¥7éq?lZN˄¤?nñ¬‰a–?œ¢ßôðù?¼Qö
2?ïE©â‰nö?{›'^NJ?}f2  ø?lÔ:&Yío?ânRK¯ß?tÒ1aáWAGN4FGL J1420.9-7920?èûˆñÀ186†¥À9ÍCÿ3QfÀ<Ќtíé@	6rWá=@±›îÞp?¾Ï8
û?ºRýRü|=?ýs՟Ú%{@Ñ
è èÃ?﫲~lí?ÈJw]¼"¿æ8ÿûÎB¿æÖT5{¿éˆݬ!¿ïûVƒšTAGNbcu3FGL J1421.8-7920PMN J1421-7920?ïm}úVȺ?"dêTP?aòøÖL·?S!f¥Ñd?á¡<?ƒÈÃîå?ï€æ/|øØ?‹4~çÛ~¾?o
g{H""?qÛ¯é:4e?ˆP^_?…ƒ`k+…?î < ËÉ?'ž@~g'u?…àⰕ³?'*0LCe‰? ":w'?Œå<Üß|m?î5ÎÛ¾"?€ÿǒz'?™[?;¶+Ï?v™¼C°‹{?Ÿêå\R˱?u	"Éwè?í¯ø‰Fü?£ÐÜÝÙ=?†:»©(4?z¼ßzêÑ?¯qÈ}ß^2?¢Ï"xzY?î"í&€ë?¤ñ$ÉLµ?ŠÔžÁì?—Lq(Ôc?¡
Š¨¨Ù?œÏ7$Zs?ì2§&lr¼?§Á=?¯ ?¡;î"º?—µR÷b'^?µÍ:UZ]@?¡ƒÏ7œj?ë ±Ìsê?—pEöùÂ?¯W¯hˆ¶?''vá_‹>?³N™éf.µ?"Uj'0tAGN4FGL J1421.1-4614¿ÅßÅ;Í¥T@+¹¼ýKð™À9ü]¦¤DÀ<
rÎ\@®ú²Ž22@ÑÕùµ?º´Fn#t?É	ËÛ¶µ@Aü#Òm@^06Ô}¿à'$,Û¿ÔiËá'n¿ãÕ2ÌÛæ¿ç›xqοïX(ñÿŒ¿ïÿ*¸:n'AGNbcu3FGL J1420.9-4615SUMSS J142047-461431?ë8Nk{´?³·ÏíÖ?¤Ë¶LWÇg?£±Yk
¢â?»×±}ø«?®Z&Ìyi?í`ßW$:X?±±Ðu}#?¡B~<¦6?¥¡ùa?¨¯î´G?£*~2#Øf?ìµâr{r'?£è)'Í1?£ÅÉÀNš?—ƉN¹D±?°n‹Ý#?™n©xVJ\?ìŽÌÖâÙ?Šv«}Ó³?¤]M´¤óü?}¥T/N™?±Zõ®=9?'&ÿŸ894?ä4OÛèý
?¿x²:Ǟ‡?¾UI%Ác@?² Ú±Šþ«?Ð
ýªÌX?»`(Ÿ0‡\?é…L¨z2 ?ÁÕ0.Ø?´Tû?\ÿc?³È£À‹Œ@?¿€Ÿ{õˆ?¶7Ýß;0Ð?ç~c˜ß=?°KªÿPô?½'´~;3!?¦"×á¨Ò?Ãr—]er?¥Øòj®.-?çîw¤Ò1ç?¢Æg_#–?·›(¬Dã?™i2w
Hd?Äx"ؘ´?›ˆÑ´ãØõAGN4FGL J1421.1-1120¿çr{[–@Fæä:§›»À9ç"UUÀ<>¨È
Æ-@"/¥	9@;û"?¼a؍bÇ?À	WC¡ë@ÿ|í'hs@
¡©7ò4»?ãS¤¢Œ1|¿Þ*߈'4¿äåZ—ü
¨¿äH!ÂG³¿è¾ó…ô¡¿ïêñ°±äAGNbcu3FGL J1421.0-1122PMN J1420-1118?ïMkÁw·¥?·$]©ê¥?pÒ$5 –¡?é@ÝT?'þÅL¸±?³Ž'÷§?︎,å!"?|n€ö'j—?]oªJªgÚ?b"Ô˜w k?|\þí,X?uQá·?ï™Z ú$ã?"yÀ¶î?ioAnÙj?yK"">GÔ?ƒM‡bÙjÊ?~ÚÆ™K?ï:kÎQ©?khE;Ûçµ?'C6Fr/?[¾A«ÞK?!Ö4qª?f6·(vì?îîÜÎïß?£¾[¯y?*N£ /j?ƒy¾§ùê?™>×=C?ŸQñ#6†?ï&?
ñi?•ˆŠÐƒ^?lh×.w@?rÞz|Ñjt?—«Æ«lø?"#DáX
ˆ?ïPù>ùC?‹}Æë'|ø?pÝt,%6–?uÑt¸ÌØ;?'Æɧî
?‡äBºX¹§?íÏÖ¾#wå?ŠKdÇǑ?™²&"z‡?{Ó$'¡üÁ?¦)€Ôg%?ƒÁ´_˜"AGN4FGL J1421.1+3859¿ÕCٌVm©@P÷27Š°ÉÀ;‹õl(GÀ<_±´B'L@Smfò'?ð´V´A¼?àœBUåå£?ïü{±QFD?øÞÅ7­w@	(ïÀAÏ?ì[Åޜ*¿î·¾b¦¾E¿ÅZè	ã¿êÎ`ÐU¿ïð&¾°ªW¿ïýÚ rfOAGNfsrqTXS 1419+391?î­õÃÞ^?£â³=gf?fõa¬pst?n˜CHÎ&É?£±M¥±G9?£!õˆ­¹?îþœ~·|??«îS£Æ7?ƒÝôÖÝA?™èD(dA?–=ê5,K|?¥Ró£î_®?ì¦Ùù䐖?¥ß@S¶?™ng#Áp?"Ü3z´YÂ?´m–hǯ?¢	R\jÐ^?íON¦p?£¿ÄCÄÙl?s"–XÔ"ô?iÓìløkT?´LAfX¢Ï?£›ÉàäOÙ?ìà霧¸?º1C¢u?zęA@ý?€'ä%³]°?·X{1Ȧ­?¹]é—Ã1—?íx£
ûZ?¿7˜eŊA?'Ǻ¿.(²?¦Äïtb?¯ñ¿×c,?¹jifãô?ê°ÒàY?«ëå¾K¯Ë?›ã	?•ã Çd?ÁÛםSý?«C;WÞ¨?ë§à:›:?¶!zÀnß?k±ÒÁʍr?qÌ𚚓?Àñ¸°q]¢?¶þg•½AGN4FGL J1421.6-4819¿çÀjŸ—E¾@'Àì1"À:…ñ7`ÆÀ;öp5ó@A- Í›@fQó蚉?Õ½1ø?⑀üâ5@	«f/ßÁœ@‹\¿ô?ï«ÝhüBܿ݉EcŒl_¿êˆÂÔ&¿é²3ž½ð¼¿ïÿøsCÄ{¿ÓÝ¥q"AGNbcuPMN J1421-4820?î!åÑç¤ü?¬7ƽT?¦ÕƒÝ¿?ªMó—¬?Œ2q‡ÐÆ?ˆq¬æ^‹?èœü;¿µ?Ã^?»×²?»•çz+?¶%VŸ]£«?À	D"5і?¼-nb´*??ë¯N¾˜ÆO?¦ù-}¥m?«:²}rï?žtaÛû?´è0Íʛ?Ÿ¼Äx"?åLclD?§GZ~jƒ?ÆÚ¢¤–^?Ÿù65'ÊR?ÃôX¬êYP?£°&©èŽ?ëë^"ӝ)?¶ÎhôAM+?¹'q çq¸?µ|¡›ñ¡?œNw%^/÷?™:÷Š'J?ÛÊævI»é?οþw¯¢?ÖèvZ"?ÎvÌ©Ö?ʙF^Dj#?ÄØR"óŽ?èWŽ0H¶í?°Ìל$K?¸ó/d¬ü?¦Zðo÷Ü0?Â(/ÐýM?¨OœŽU=«?Ўß1åfˆ?«ù9 äÐD?ÚÆ]
áÊ?·ª›$­57?ÕmZoüÖï?¸EH´ç¸<MIXED4FGL J1422.3+3223¿ïýCŸ^vû@Qh~AN~éÀ9t‡Ù}µ8À<n±lôõá@zæ'Ì@ù©™èt?©úg\'¹?§‰ÎÒ`‹?ùzà…v@·½WÓ|?ïÿù³>†¿ã€!ùO¿æXÞW(Ü¿èwhð?ï¿Úgéek•¿èg˜_ݶ)AGNfsrq3FGL J1422.4+3227OQ 334?îÓê'р;?¾ŒÆÍYd ?O²à€»?j–ËTmè«?¢B"C+]X?½ðwÕW=‡?ïãŽâ^.?wM¦1°?5åyPÞ.?B"…¼‰Aœ?i´nè9ô?vwÔFlŒ¢?í•Rw¨q?¥Õçë?^‡|Î?8.?k_ª3<'Ú?²ÛNV
‰Ø?¥½£Ì
å:?ïþ·ÇhE?H·Ã3a>ÿÚko>êßç«m(¥? £N[aÇú?1êÙá1?ïhI.a?´M~šo{?EÍÂzþÓ\?S&±MHí?ˆ¿›z´?´/'BH«¿?ï¦DÛ&V×?Œi
r)?J_òž½û?Wø2fd¤ú?"ÈØF^¦W?‹‹UŒŽ5?ì<¶}Æ&?°,®Gœ8ë?c·cTt7?m["	W?½|'Ì-?°,#%rK?ïü&"òÉi?2V9/]F>?"Á|Sæò?"²_çN?8ª)ì5Æ/?0€¶êAAGN4FGL J1422.6+5801?Ð÷«a†ò@K›<Ž%ÈÀ:ސ†Ë`¼À<˜Wk àJ@ Ü}78P~?ö$‰íT+Ñ?ÄÂ'ϨŸ?γõ:,Ü@
›Háa«@I×áRëµ?ÓT^¦ÿ^¿ï'ᐩ0?åôB'KÇ¿¬‹Ü"à¿×éû[Ök¿Þ²'#ƒ'ÇAGNbll3FGL J1422.8+58011ES 1421+582?îÛÕ.MÎÉ?«‰$cY
/?~#åf7sµ?…yê¥ñXØ?œü`Þôÿ?§nž•u?ïqqÍwÃ?¡…aW¢˜
?l$£5Â49?ƒsÐN7ù?Œ'úŸÄH?š)lxÕ`?îf‰£ú'û?™ßžq?'sõ'‹?Áۈû‡? Ýk4ê3?'ñòÔ 
?íß)YÉ?±©'[>´?y´'$|¢?dÊC³›'Ù?®ìg¹ûù[?Ž‡þ9÷à†?î‹è…ÝF?¢=ÓšÀb?…s$89D?Ÿû)IÙø?¡ä®'‰ô?ŸNX)lú?Wé½?©"kAšé¡?|y»ºÓ?‰—ÇIœê?£¸Ù7Ú±?¥6y9¬èå?íbK÷FÀP?ŸøO¼¾¨@?—•ø'æ­?"Ü*Ë¡"?®SõŒ¾Òª?š/|Ð?êÿ[ìdî?©	Æ»J?‡'T•r\X?'/ƒÚwP¶?Š‰H
'C?¨ç2<ˆßrAGN4FGL J1422.6+8150?îÂGd²K@AL\1Y>À;¹$Øý\¸À=\-þ@@©¤æ©Â²?õ'
0Ûj?á4ڂ˜?è•Ú\ØH+@»7^;º?ðuR½g¿ïÿb`ÈAÎ?ïÿ|Ìy?'ëËRÔ¿àÏ8·×rB¿èqgù
¿ïÿþBe«+AGNbcuWN B1426.4+8205?ï'£¹¶£?ŸÂpÿý?ƒŽY"ñ?•¼¼Ÿ&?"Ed{98.?–Ý%م!O?ë§QÙo%/?¾Kôl›V*?³ó2Óì[?·ó¦§rjï?­¤~eeÔS?¦™4ÝÁâo?ìQX"/',?¥ïŠ7¸`?¡k±2uD¼?–ŸF	'=e?´¿bÃþùÄ?£"zÄ^(?é؛U9 ?¤ÙÈÌ¡©•?·a^b]?¡Å(ß4gí?¹ÙÆõI#?˜Á³÷»NO?îYév.c?¨àш±ã?™VÛ'/N4? Có"þG?›kö
Üä&?›ar?ç,¶%…9?É®óáY?ÂøªSÙ¤?ľðéëO?ÀT}ë´?»™;ÃÙÛ?ë)ð†nD?ªí*'àá?£ö|b|?—34A›û?½(Ž\¥?©cenÞsØ?ç¯ûŠœÈð?±iòjk»?²m=e!?©4,"kç?È4[Jî)®?«3†Mä×AGN4FGL J1423.1+3738¿Íù2dñŸ@Q#_€™À:îؐOÀ<JãÁÛØ@ýÔö¼à?þ׶»%?·«u#I?€¸!Df@	ŠC»@Ò÷BOù?àã;z)'¿Ûþ\;ë¿ÞÀgmÍ¿ÝR•äƒLÑ¿é_6&,ºs¿áš3½œ®!AGNbll1FGL J1422.7+3743NVSS J142304+373729?ïñ®i³<?M=;F
–?Ibƒ×nڙ?AÀĜÎ{?Oå*|DÖV??Rà¿îL?ïá¤ÕYZ²?l–K‰}Ü?@;)¤h?I‹']È?jL`l+–??h^K'dêª?ï"$G]Ê?…OfP´%÷?n6
€™?xnØw¾9?ƒ©k|Xs½?NL-p÷?ïïå³£†?@¯+TB—?2E¿—pDè?éÔí&…?[£(mð9?>~Q¸Gˆ²?ïâ¥ãã?`J:ÛÐû?`\MòõÖ?V׶¡nz‰?YûÿjÊ?MÂ"žº?ï¢ão"%?"Èʁu?TÇû½h?aÿÛ×K?"áǵ՝(?'šBT™û`?ï(Ě׺Å?Ã
T~å?€"ëîðH?"m<ÏUF?'¤ö¬à—\?‰åˆ'{ÁV?ïÔ}w=èÞ?`6 tÚëo?GyŽH«š©?6u"-¬×[?rÒˆ£*?^5¸Kpù¶AGN4FGL J1423.5+4524¿ä;UcLÎ@P'û?¦ßÀ;>eV›îÀ<å'ê)Ôæ@§$íË#@‡±¥)Õ?Äßʇù¿–$ƒºVŸì?Óâ:\È-@K>ôŒÚ?ïÍ8ÝŠ¿ãà'ód¿æ	ˆt®'Æ¿ÙóÿÁ–¹¿ç-ß×kŒ@¿Ódƒ7W…"AGNbcu87GB 142138.0+453705?ï×öáô&X?`¦@¥¿l?D!÷˾GN?3Û8"o)@?q€P2Sç?^l9z"?ïÀq1?t—BS|?OÁP©'Ðö?TT´"j2}?{Ï=M'ûå?qúé<j¥?ï€þDééé?t¥¼FPŸ?_°ŠÁvm?EúÊkùݜ?‹Þx¼lfâ?sk¸?ãùò?ﴔZ5y?]…¶ˆž¼È?fž>î?Fƒ(‹Ån?z¯ƒç±Ï£?[}iv1þ´?ï­ÓÀåkˆ?t3Áy¯³?R³ø|ÀPV?F‡ø×g?'4Â»¿õ?rÒ?FÌ¡?ï]2[O"?Žÿ´Ã¦p?Y×±wœÇ´?`«#ìۖW?'¼9yá0?…‹8?ïÈR9?"6 ž;6?k³Gõr?^|Z`?œ{–¦û ?'ñÛ²@d?îý*¸äm?|õÛAَ?TBbç?g(PA9è?—°`Ö:¦ó?{¿L0n)AGN4FGL J1423.5-7829?îÁûç'ÓÀ0x,äd™À:ŸSÌ/îÛÀ<,ƒ2O¥@ö€»|Bq@8xñÝ(?ÇŃ»5÷?ÓscúÑAü@	ÂsBûÅ@Úâ9E›ì?Áùß?>¬¿ä¶Ñü·v¿æ[`Fþ¿ãMf H	"¿ïÿôÕ÷?íx= ™AGNfsrq3FGL J1422.8-7828PKS 1418-782?ïÆ»ëu{Ï?xâyo &?a§ˆÂI×?dà9}Ýuñ?sÎE×%oi?s)Bûo{?ïhefƒ?"ÂpPÀ¤Û?d&N\4?v'ig`?ƒœC`³0?Žˆ÷ìW?îUˆ»®tü?š'­ïIÌ?'jê?h-¸`^?¡§>ý#©>?"›ÜÏU<?ïzãjÀ_£?pãâOWa?`óŠÍ‹%?I£®öG?
B¢\£Ô?mômY°"œ?ïªëâmÃ?{¡­Bӟ?iåþàB?c»Ø1Ԕ:?}—ùÃb?vžWÇѶ"?ïê%ù
ó? ²0õXk®?y'•íK?ŽVÕë'­x?—ÂòW6M?™_€öK?í ~)ž~?¡qkïež­?š¦Î'ÑÎa?"ŸŸCÜáˆ?¨¤¶$·ð?š;
®^ì'?î
Æډ?'Å{H…ˆ?|²Ã{'Ý?i ó.¦%­?ªy¥ôñ¯?'Kûb(AGN4FGL J1424.1-1750?âûWî9À&@CÜÛ7ɚéÀ:³Ú°À<ixX×1«@ œ­çYk?ý&Á½¥?ÃÙjM%Î?¶¥"Ÿù@Y?ô™6Òúä7@
ŒŒ÷¿ïÿ;ÒDÜ?ïüé)ú¥M¿ÛßÚ¾[¿ÞÄÑ ñý‰¿ØI3$Ň3¿á>—jjAGNbll3FGL J1424.3-1753NVSS J142412-175010?ïõk8Հó?H ÜõTDº?#=Û¬&šÝ?	,&c"?RÁÒwK…ù?Fىõ¤{i?ïç¦mp#‡?i°%oKÍi?7L¼ Rõ¿?Eh!'F-Ê?eoû86§ƒ?eê¬SÝ?ï³öÏL%j?tP•ó–y?M‰6¼̈́?6u 3ÃÒ?)¸½K§€?t!Û"J4±?ïÍÊ5MÈ?T""©øf?Fû2gž6?+'YñÆPç?v;'ß,Cª?SÆQ¦miô?ïî¬VÆÇ`?U"?4Õ™?-š¼CßÁP?]vŠHŠ\·?S&M™~R?ï­ÉE‡Õ?sdá·¼?L†ëù3ú?VL˜ºÄˆ?'Å?æNö?¯~ú'Â?ïm-®±Ñ?ƒ‰
Aܨ?Ued
?H´-A[?'	ÙNŽ¤
?ƒ/L¾Z?ïƒk©é•R?rÀ›Š6?WÑ
²«h?FÉk^+H?Œ*ôw³?q›ØÕ AGN4FGL J1424.1+2917?ìË9sX6@Q`ô^NÀ;ólàÓêÎÀ=|ñÃ&[@!mÇÏâÖÏ?úA×:äØ\?Óò۟x€Å?¿ÿ°ÏÁí?ë)À°3å@œÑOŒÊ?仪›I¿ïûÕÎÔ
?ï+Îð"{r¿Ï<ÑW "_¿ä.Äf¿Õ
5ã盅AGNbcuNVSS J142408+291800?ïàFï)ˆ?\­ˆì§£h?8f"ð;Á¦?-c¡ '™Ç?l¬LŚšF?['°-dÔ?ïžÍÌׯ?‰'¾Är÷t?Y£»3¯ÉI?bCXañW¶?…¥¢Ÿ#?‡7®6Žù?ï*'?éW¦?‹œî¬©=g?a×QT}™?oˈ2͵f?˜tÍۋC¥?ŠŸÉ3%R?ï_´Ê2ÏÇ?uår¥ë?`­ã†ÚE¢?S	¿/M?'óªEßi?t|>-Ñä(?ïÂS+v?qUöŠ–?F¡vF?@<ÉÖ>Ê?|X¡Œ?q
ÀKE	?îLjUW(?³˜ýE†4?dCì3²n"?raÚ@uâ?¢C;ä¾£B?³S)|Ä?î‡L²áV?"û²ÿ¡T\?gGö¿‡h?n˜†'b?¦µf8J?"ŽÛæËDš?îX°‰u4?"ê89/á?k??…üÙ°?iGYÍZ?¨Ëàú½\(?"eæ?¸ÈKAGN4FGL J1424.2+0433?íq€'Æø‰@M3•1ã¨À9ÚÃvõØÀ<(9oV•@Xlþ†c?ÿ®Gx?¶[²Ù0³Q?ÃLßV½&@4±?¨Œ|@­¡kõò?ïGŠ¾4ƒ•¿ØÓØDO:P¿á3§—‰!¿á'­"ãY׿æå>³™õà¿ïÿôw5ÁƒAGNbll3FGL J1424.3+0434TXS 1421+048?ïïø<€þ‡?efšûƒÃh?Eh©Oq'/?M.Y¡0b±?U[2Ÿõ1P?]ïøú;ë ?ïâöíÔý?iÒ/ò:â?AÐâr?Gµo·Y?i"ýxz?eNvÿ:†,?ïªÓ‰ž/?|Z
½Ÿè?mÜ®;o\?v&¼^÷?{§ä$øû?nCÉŸ?ïäH؝ É?Kšâ
?Dö:0·Ì?+Vá÷Z"Y?fy˜žýµ?G ù¸ÊûÌ?ïíãa¨€V?WÌíWQŽ?NjzéNA?FãNT?U8"-"ë?NË–Ao·?ïœ?ðʜ¶?"¼Ú¥ù/t?Sÿ†N¶`î?`øKÐ4?†pÿºt€?'åèž&?ïp
®'×?†&öË	9v?yÛxŒ-Ë?ï(́˜?‡oîHŸ5x?y­;ÌÔ?ï¼kϤ?f¹{ÛDi#?W:×'ªÐ?E<ÉUÎÂ?|
ûlý—6?dá ì÷ËAGN4FGL J1424.6+1447¿Ã'ŠŸb0@PBçÀn¹À:iȉq-jÀ<uÑá߃‰@äk*Í^@7ÆZÂÄ5?¾G\5
"ï?"Æ4=…'È?ח-ä>ÙZ@
ô(Ü¿æ˜\þ2ËY¿äžOv_Ø®¿åÃƓͨ¿ÜTF=Ñò¦¿æÄ¢t´³¿Ý/"—Ú|¹AGNbllSDSS J142436.29+144910.5?ïòX¿Kt?ovˆ¤ªý?4{É	|?FÍ"ƒÁÀ?V11(~'Å?jR'\ˆ?ïá.+_e?qTӃ­™‹?<¹BõYxì?Gm˜cˆH=?k:քhì?o§'A!T?ïÄ|@dÁm?n~ï¦kç?PÀÐrÒ8$?T±ËD,™Ø?y'«Æ8OO?l`¸[Œ|Õ?ïè0d!Ä?Dт:H€H?=uaÈN?!N+©@5?d ï›"?¤?Co,€+ÿ?ïíQh8´¹?X@ú`I¼ñ?;pìw(c?3Ã`?¢þ?^€ô3º7?T'Ž×®†?ïÏ~Þ?ŠêôCøí?J^Š¸Þp"?W°ÜSïë‡?†æV£µ-G?‰ÂWØøâÒ?ï™~©~>?x§]:ç\C?\!Äê`÷‰?dh0{öƒ?†û•5|?uð ®y
?ï»s?e,0:&?TïKOÏÃ?@`ÃQÀx?}
'Ø(y?c"åuq8€AGN4FGL J1424.8-6808¿ì§Øä³yÀ]{ý§`,À8ÉBÇ$íÀ;€нV@Yà¶Bó@ç>?Ö¯¥?«ç"w³?Ì._6qV@%€Ãÿ@:Š*»À`?ïõáμ'¿ÝU|o?¿æ	àž»Âc¿é#™7t¿ç|}Ê0:Z¿ïÿ/¨;ôAGNbcu3FGL J1424.6-6807PKS 1420-679?í«Ï5K«?´H±äÅæ?¤Œ'è"?³Qr±	?¡:"8?šÈ!<FÊm?èpª‰«æ?ÉEƒ|¬Ï?œÄ¥	Zï?¥ÿÌZƒ|?ʧX´w‹?Æ­7Í­?ëÀŒë
z'?©+ʾgŸÆ?±ÚSh\à¬?¤‹±¢Å`?°!E>pÄ?Ÿb '¹?ìïhO—?—‹uϽj?¢¬ n Í?…{|ÛÅNƒ?¶)ZuÐ
_?'`¸d{xÉ?í«&·Z?¦dl‹›?Ÿ9ºg/Ü?¡+°ÿ(Á?¥±Ðœ5m?—û{ÉÀw?ãNXÅ,ß?χ㛒ºz?«™^À'J?²w¤¶É¤?Õð™u‡kš?ÍÍcôNÏz?êu¿ìƒe??­W«&"?¶"[ÃÕjF?¦b'Ê·,?µ½¤Ú5-C?£ó
Â.k×?åA›¬?«;‰fB?›?»'-7èñé?ŸÚâ›É?ÍfdÿÅ-Ø?§qÆtv¨AGN4FGL J1425.0+3615?é°äÂóì2@Qn'"šVÀ9؏AQ(À<
v{‡`@ SEµöâ?û€ û?¶ØÐç
À³?À,2ñÅ«@YQûuVÄ@TxžÍ5'¿ìâT1?î#Cœ7̿ʸÂ~À$¿×`½,à¿à±Šâ¾w¿ßIà>¿jAGNbll3FGL J1424.9+3615FBQS J142455.5+361536?ï¶$	–ú?r~ÿ¾'t¹?eÔÌ2挲?bšsX?z‡áÁ<ª?iwaöe?ï<'©Vê·?–Œì¹±yü?€…í_ªb§?‰µgØ
Ö?,´f]Ñ?‹S³£‰q(?îÔ®D:[_?Ÿè~?‰`åå?‡ëf­îl-?˜º7ƒ'G?‡†±þfä?맵‡r
ñ?"ÔÕ±'+"?©!ÈÝÁ÷
?‰e³6ni$?¶1oW´nr?Ž"¯ÈG;…?ïeí@pï"?ƒÐ¶ƒåžD?®"mûv?x.^I"Ÿ?†­f1
¯ž?v÷¸l›DL?í¸(a.Tb?²Ùt ÇÓl?—hìli#Ÿ?¤AXùŒ
Ÿ?¨É´Rs?§TÙ;¿š?·#»?šÓT–ÔD?'ë»vú?Ž—þ¾Šò?¦ŒôÀgÖ×?"𙤏?ç¤SÓ¼M?¥¤Ì匼Z?¶i™/h,Í?œÁbþ€b·?Æ9ç]Øßf?£»¿ÕP+AGN4FGL J1425.4-0119?í¤
}ºô@JÒYÀe¶=À;lœù	À<ÇÏï–ü0@!à*w¢Ï?ö¡›Lø?ف9ÜÆÑ?ߎ0Ú¾R@ŸL{ٕ2@ˆžìää?ïû°&äp¿ïÿùëñ?ïþ¹ä'¼0?li|Š.¿æm›¿8º‡¿ßõ b‹AGNbll2QZ J142526.2-011826?î±¼ñÁ™?º¨U+"?_—4Ù8?uoDi	F?£çwEwQ?¹Í\zæaZ?ïŸL#͘,?†‡Z…ìð?_"žläó?fAÃÛÑA?":ƒ//"™?'{»f¸¼?ì†Ê‡Ö¬'?¯}æo<!9?hÇ°‰o\ß?sIӗoy?»n<§-ß?¯Y‹©ÅJr?îõÒ~T?ƒŸbøp;?jÆõÈöR?WÜ¢ÿ­?ììNˆ©P?'àýv"áè?î›Uƒóž?°ÐOv"bÑ?acÁЭGš?^l‹üÈ?¥7î‰Ú
­?°³7Êy?îé˜ljXÜ?¡Ñé°Ý?vS4RÔ=?Œ˜"'(<I?8%v·5o?›
À"Ò‡?ë0B'÷"?±š-Ž¾?d÷ãÐM?l¬Ñ¯jž?ÃG_i`Û|?°ü\©X'W?í¥A±-èy? pyKáØ?rû?›0Q?mæiRíIW?±´2¸q? MmWWòAGN4FGL J1426.1+3403?àðo&±ù@Q!灃ùÀ:Kñq…À<˜Y¸Øú@zã ùµ@ÓÅåQÿ?»æþ§:l
?¹
Ùͼ5ü?þBu
n@Jzpßf-¿ì
þ‹¶­¿Ö6j?Žá/¿âYÍ "¯Ó¿à™_æÌR¿ã/\äÝdË¿æ@U$õ'ÎAGNbll3FGL J1426.2+3402RGB J1426+340?ïçÜËaW?QM&[Ù{?EÀþ¡†®Õ?2‰êpVW©?bþãÜ?N!ú+Ð?ïÍà'¶Ý]?vAä¯u+¯?O½å\㹜?Uø®$¥4?uúkk0ï?r`?XÒ?ï¦3"
¾Q?s»4€›u?X«æ6?Eç£;Âý?ƒcB0ÿ?rí ‰HLÐ?Fª3p?b€^J;J?sz¯²)oO?T¯µ•›¯?€{VŠi?\!¢e
×t?ïÓ?Ȃ?aÿÚäè'?T€óV¸—5?B(R2‹¾i?q@B(".ª?_ìVuš›S?ïrÜWžf?Œ½ÂRC›?`'£~f?h…Åþܧ?AçþlÝ?‰cz´c"?ïe²và1.?k]fxˆ?dE¾x
¿D?VšûŽÂ(A?ÀùO¤½k?|‡D1ÿÄ?îîÿuô›?€*'¬"¼ù?ˆ‰èÇ`C?p´3(Äjä?•Û(*!®Õ?z¡*a·ŒAGN4FGL J1426.4+3625?å[¡TµB@PõöM½ùÀ:Tغ@ÙÀ<F<"¸@/fRÅIÌ@A'Ã'ë?¿
SO³F"?—'(6êÎ?Öˈü@›©×Te2¿âìËð¦¿å:"yÄçü¿ép÷б^¿åË¢Ëq'ú¿á­òKâV¢¿ïÿÀéz-AGNfsrqB2 1424+36?ïÊ>/ā?q(`b""?YÀþçù¨?KNòY«¾?tp¨N0A>?o'™>?ï֑÷[8,?tgpÅlˆ£?D"¶'KÑÓ?Næùuíq?r$mŽËú³?rJª²Áiß?ïJ‡.¡ÂÍ?'ч`HÕ?nÓ½,­õ?höÎðâ?'Ô·L¾çµ?Zæ-®}n?ïÉ2Òíæ?[ß0C>?^î5µ"
?FÎ	‹K'?s«	uv?V™1Ftl?ï‡~à–êN?‡Zû ¶¨?ksR¸§ò?eS"å©·?‡Cs+͌†?"…ƒ0MZ?ïr}¼Ø?'᯹¿Ês?Zˆ»K(F?cű1'?ÂP£Ú±?'åhYm ?îg›g?'¦m®?R¶ŽÐpy?sqã¡íQ…?£ÿ/uŽw}?ŽìŎà›?ï]ㄎ†?{<#^4Vß?xÄÉÀ ?i&@\ï ³?Œ%m¦ðœ?u–²\|¹TAGN4FGL J1427.0+2348¿Ö
Áœdr@Q
´·,À6Ô{Ås<8À:º¿&¼@` ãzcH?ûHcF uÁ?Žec~võÍ?­ÃŒ #$â@37ÿJÎZ@Á¿}ƒä¿¼Fa
a"¿Ñ˂Iñ»š¿Úú¼#\Q¿Ø"a`î{¿ÞïҋR¯¿ÞÖ-¾ÕlAGNBLL3FGL J1427.0+2347PKS 1424+240?ïÚÆ#$è?l/÷¦T'÷?B9¶'f¤?Dê®/§H®?pU·Šwë?i؝üWça?ïi诉?"º|ŠŒ'Ò?pqEзB˜?Ü'iªƒ?M1Sb'A?®ñ)?í†
~'³û?©Kþê­è™?†2ì‡kN?zsæ6Q?±	NxjD?§W-¾s&?îǖ³qm<?‹"X‡·Œ!?pêZm€'?Yد€ù÷?¡iRþm=?‹
0Ïc|'?﫼"tbí?}^õ>?JÖ.DëÓ1?DQ1"°/=?ƒc"v…r?|?O`î#?"
M%?§w§(éÒC?~Ş©O¤k?úxׂ2u? |'üVú¤?£Ø¢°þìÙ?íª#(	o§?§‡Ñ'{»?~¼¬DŸGÖ?…9Kî ?°Ãý`?¦øQÛ í?íÄõ'Î{ù?¡]Ð_'?z9i=]ü?n𛙆á?°4½UÜ6"? ÒxϝØ0AGN4FGL J1427.4-1823?îã\)€@Co`|A™þÀ:_'‰±ÅÀ<YðHÒש@ l)lŠî?ý&ÆÞOâ?Âɋ9Y'î?·õºgš?öVuÂú»ó@žé€â"‰¿Òº|þƒS1¿ì¿"zM£ø?«p=]a7±¿ävH@áqŸ¿ºÝå_&s¿è1D±	ø§AGNbcuNVSS J142726-182303?ïk†Sõ(>?Œ"£5…»?Qüπ§¡l?Ckg˜'ñ?'ohŠÜQ?ŒÅö6+?ïÂ'¡jÚ?wÄiÈ6ã1?P_˜­ü-Æ?U̹¨Áù_?zà…í¼oÖ?t6ÿbϗ¨?ïtÌR ?Œ¤Üæí$?eÎ.Jbô?eè7aÃï? ©¯ñˆ?‹³ÆÜì×9?ïߍ]í?vyO`á"b?a®öÇuá‹?Kœvæc?›®/xŸ–6?uà‡¿ÿkO?î…#Ü0˂?£n›»W»?h}¼	VN?_›~j?¦%æzy?£)šn…ã'?ï^ägën?Hy'G'Ï?`Cç	ˆÅ¯?f-D&˜?'6Ɛœ‰?Šl ä§å?íØj©…ä ?›Ò×Ë$ùV?s9…ýAt?p‡ªçqT0?°	R†îC?›CøÖª–ù?íy÷Èy?"®€iC{Û?rW"Ú¡°l?fEè@=D?³
Èp¹—?"U¨Ä}õ"AGN4FGL J1427.6-3305?˜¢«4MnÜ@9–r§½HËÀ8ŇB_ À;Ȓ%1ñ@B†Òeh@–'³ÌJÇ?¥C8cõ?¾"yNõ†@¡aä÷f@SÅm2¿Õ©ma­D¿Ö¹ã»üšñ¿äe0Áhë|¿ærᏥ¿ål¦â,…o¿æ\_©÷AGNbll3FGL J1427.6-3305PKS 1424-328?ïëèç	¹è?W;dékB?HëwZ8ü?=éU"?[¸£Â^×?T	cñö?ïÏO Nª?€
t-'u?MÄ
môíô?_ö̂օÇ?tŸî¬eN?|Óö•¨³:?ïTpŒÇ?'K¿*© ?vÑÑñK?€è‡æÛ@)?ì{¼—?Œg+¶¦À€?ï×KŒ	?RŸ3"õ
?Qe<©ÙI´?56 öAˆ?p$)¿'ÜÔ?OÞ·5;}Ä?ïÖ¥§€X?h;`¹?Tµ÷ä?T*
·Ñþ?nÿÍ3Þ¬"?c©þg
è?ït£]	<â?£n5<Í»µ?g´ÙÂV?…bw–Ï
?Œê"q4Ý?+êŽÂ=?ïS*ù4?e¡¤½Õ‡?sU¦3ˆ©?}Àq¾?›?ÇQ2®›7?Œ™«ùv,?ï"
ÎA8|?qÖ« '¿-?fúm‡«z)?QùƦ}7Ð?…}ñ
|?pEçi}ìAGN4FGL J1427.7-3215?ÚªãU¯@:X_9K{)À:-70îµUÀ<C¯æâøˆ@¢Éübç@ѽaõ¾^?¹ô%j‰?pGڊ$±?·­=+H@å?›\'?ɛj^˜'¿èO¯'Âe¿âPmk=e¼¿âT§BÔ¿ãÌ'áE¼¿ÈÚ*~…AGNbll3FGL J1427.8-3215NVSS J142750-321515?ïñV{P?QuŽtòK?3¸Íük"?$Z´ßlñ?Xe	hå>Ú?O–øon…¨?ïå*£äîy?pÔï•("?8Þv)`v?FòÂ	-?g¹ˆÉҙ?nÿžN"ŝ?ï¶Ã9a[Ì?qۉÓ¶B?Ok…Áž˜Ö?7P2jÇq?€XyD¸·Y?qšõ.SÇ?ïÚ²9x?P¨ÌÂ7?<:Yú›d™?¶(vý‰?q2b»>	?Pv®LJ¸?ïåÿ|ˆ¢â?a@CP•?@úä*ÊÖF?3¸™ñü"½?eÁÊl͗#?_fUÀƒ?ﴂ1õ'?"®ù;€`?G€ˆÁÂ
?Uý¬çÖ?gW xwŠ?ƒk'8U¼?ïhÞnéJ?"¿#IŽÇâ?W4ø¾@å?IuO›°?'‹ô«¾(R?"R‡êv'8?ïŒÜ "ô?q8t£†{†?Tóòs'7??b¥2Â&?Š*Y}œNZ?q:Š$¼AGN4FGL J1427.9-4206?á š(4Ò@1DûC؜åÀ5µ¥BDH.À:'¨æ=·@áÃ;Ôl~@Å,?#+~?}P>à$=X?¶­ÿ7¿E@1tÿ†]}@#ÐÜÑқ¿Áã¸á2Š¿ÝÍ+—]7¿ã¢U_­å¿âÿÀ?Ѐ¿ç¡¢4¿¿ê¤0+@öjAGNFSRQ3FGL J1427.9-4206PKS 1424-41?ï²>ªØ?~×íÙ%ã?WQu0‹:•?WÐä<Š´Ì?€Ï½åJ¿?|fo'3p?퀌º/ˆ¦?ÌØFŽÀß? >üì¯~#?¸$§^$å?§¸7mÄB~?º'€ñWÄ?칝eV?¬žsçç?Ÿ­IÔÔ:ý?™Ÿƒ
r ²?²GÂ`õÿš?¨KcœîÝ?ïEæeòo–?"ÌëKU"?bð''Ì?[[Œíà€?ŽÔîlJO0?‰˜Ý/f7&?ï#²w¿‡È?—IïKøˆ?dƒ#jÑ ?e½Ek}%<?™	¥YzÌ?–hýÁÇ?ëS€È½H ?É&ï`©Á?±])gDn?ÀÌ9Зm×?´и@ƒ?ÀÃôл³?í/H¸*©L?¨¯¥«'ï?'4Z'­-?"‰Ý|	>?±ø£›IHÔ?¥-…4·á'?îõ…?¨ŸLeM%'?¸øéèè?ØFŸSo?§rú›Ø‡B?¤"$J3ÁAGN4FGL J1428.1+1629?ïö³_µ¿Œ@PMØ/×^ À:EçjÝÄÀ<UŠ"C"@ŽZ"Zî
@‡ëy`>.?½?s³VB?½ËÓþo\.?ûöÚ7›@§EaE•?îäӉp#¿æ2-¿€Þã¿å¾Tdc¿êß !s¿ê}'gv0ß¿ðAGNbcu3FGL J1427.2+1610MG1 J142813+1629?ïãGà¿Gÿ?d"ŒM Å?P'!$¹Ì?H®ìÐÊ-?doŽÒBü?at‹.¨"3?ïTšó(?'óébïÍ?fҀˆ?m¸<´F²,?ƒ*$¬]Ǭ?{mfT,±?ïržï?ˆÒ² îÐí?o=8'@ú)?xŠQãJ½?‹«*)Ž¯?ƒûkñ‰?ï<&zÖÏ?v×Ð?TÊú?àUüÇøc?rþj¥Ï€±?ƒt›:?bßbæÔÔ?ﮥc–F?z°ê½ÔY…?f*þçm8?_µJ¼r$Ë?}—ÎÜ#.g?vŒd8?îà¤^ÞK"?ŸÑÆÙ.4:?~Åè1£*X?ˆ¨ÐË]m?œ9úNbï?˜
ω7=?îû°ø}L?KW)M$x?xˆ~^Yñ?|aÐ}"ø?šzÆ:yˆ?‹°Ì‹ëMo?íÊ>C?"@0Ø̱?¥ù1ÀӀ?'>o'¶b?šÍ³OÔþ?€F2ôÞáAGN4FGL J1428.3+5635?Ïo—§üÞ¸@Këæ`ɊÀ;rrä#+À<€ß×@ϔ*ÄϨ@Mv«Xÿ?Ñj;<ìðY?ÃãC]©~?ò†	êdH@Pÿߞ¶¿ë¦ %9um¿Î›C踿ålZÁ'œ¿æ£ßÙj¿ïÿb%>Ô?ètÛߏG0AGNfsrq87GB 142651.1+564919?ïâ›WM³?bÖ±±h?Q{¬Ü0á?G†Žõl]ó?d¦Ò{.<Þ?`'F†RÈ?ïÁÐCh¤H?{q€6K_ˆ?Q˜7¼ÖDÑ?YVÅå¢
¶?z±ÐB[Bê?vé°¿sÈ?ïSéôÐÌâ?ˆ858Œˆ?l×FÃöÉÒ?r+9òn?'ç؉˜?†‡00Uz‰?ïྲྀP½?N—™°`?RüÂzbÄ?8šJµB.?fýîñi?HŽªjè'?﮲¸yƒ¥?|12uÀ÷?c`I±™Ôt?_ÈKÓþóM?~ömƒQ?xq=ÃљÅ?ï*IՌ?¡ŒsbŔl?h%ÙU^½¹?¦b¨9?—²
d?ŸH·\€½?…Ö2?"B©Ì+b?tùŠšù*?u°¤§"ˆÏ?¡ÄÖL<Ž?'ÀËi?ï EªP˜k?qÇj)—è?f©åHÓ?W'¥¦
ŸÐ?'kk0— ê?m—YÆxïAGN4FGL J1428.5+4240¿àOšSöÃ@P9©¨–hÀ9t"à4êÀ;ÿO†Pº@!¥ÿƒƒX?ù°³â;ë?«6ý[ú–x?•'ßÿë™R?í?jCj¸Û@f;¥¿é1•Ùñx~?èR€f­¿Óù
'åÍû¿ÙL;l茿ÊÓ¤—Ïj¿Êß"$m¹AGNbll3FGL J1428.5+4240H 1426+428?îïI‰‹Úi?ºìž[€ý?k•ŒrØMS?‹jkG|(?ž¤Hh¹"?·ãÃ:¾$?ïÕÞ²Ž™G?sm@¨M9?DùøR"ç?OÜÜ҆â?rqgº…?pû(±£FY?îás€*]?')¬k%?bùÙëxô?dЕ2=ª? ·gØþʦ?'Ò!$±Èâ?ïËÓ¨‰!?v	ÎØS?n MûÒô?R k΅ä?™Á~ó¢?tLýùkŠ?îZ3µË:?«Ü05/•M?t_9Ü{?y)ƒyúp?§Þ*ûÓ¶Ñ?©ŠkbÖbC?ïˆÈÆF?Šä¶p?Wr
k|ëƒ?`TaE."?‹LQvÇ?‡¸cÙ8â?íßË9¤¼b?Æ {ðm?lö šŠžj?pãŠ¸'?°õ+öü?}£;P[?îƪe?ÍÛ
jKª?~紒jç…?k²è®(j?¬"=
CãÄ?±hÝZAGN4FGL J1428.7-1017?堄gáÄ3@Fà:S¸ä¸À;I|­ÐˆCÀ<œFÙÙ$Ê@#
‡þZä?öõbÓ3ï?ӗ…"P??ÑI¬|]I?úèââ¸Ç\@þÁFÆ8¿ïÿT_™?ÝN=»!~«?6Ã
¬?ÜZ'±m˵¿àn¹ª?¾ëƞE·AGNbcu1RXS J142844.4-101801?ïág‹Õ`Å?]™VŒÙ^­?EìõVSda?71œâ=*?i6ô=<?Z®€øã'?ïΡÚz?vñ§k.ñ?Kk©àɅ?X픰33"?uBO	V?s‰ÿÀÿ?ï"ã*˜k-?"¦•«x?høŸÑ ?m•H—?—†?˜"†Ñ¯¤b?‹Ä1]¿?îïÎ"'?…K??f["Âq¬y?U–Rtd~v?Ÿ:Ëd	B^?"Œ)½•V§?ïÆD#‰r?s'q;µ?SW^U\¾?FŽKx±²?x"|ˆçó?q¨î'Á%?ï^n^Ç$†?–OÌÀWÄ?gêÎéeì?Œה̷E?'4ð&âûŠ??•œT?îŠj­{^?•KâuŽI?rjšr›t®?x'![ê"?¥ÝN?"ǵöAqW?íx(Ùú? ©E®ó8?uÍN¦ þ?s H7æÇ?²áäCÞg"? ©cg¿öAGN4FGL J1428.8+7429?Áº²ðúöÎ@D'À~áÀ;s֑q­À<ÿž)\ñ@!}@¢‡~å?þË׿o8?½Ӑ¶¿¶s"ölƒa?ú{x| @	#pš…?ïâ½—¥¤¿¨nâXFµ¿æwÂ,ém¿â°â`‡Õ¿âd ()ö?"cþ	äAGNbcuRX J1428.4+7429?ïȟ2­Ò?•D&¾†6?7¿`
¡x¿?7)6UÅ?z4pÇ~´Z?•>	€%b?ï¼'Íç?zB,·¤_±?Q^M8{J?VÂëœâu?}›âWü%ã?v[®"…??ï
%1àR?"ʐvI!K?R—)¡"ÝÄ?\•uõ?'ç)·ŒÞ?"À–SV"Ó?ï£Ã˜þ?tGÅ{ɞË?a¬õuƒ?JæH3ùiQ?'¤9™ mÓ?t +ýW¯?ïÒ7}DÏ=?}'
ùeÑ?E»ÙÇöf?ICËR
É\?t,Æ3·Ü¶?{á7©î³?ï]Qcí1¿?˜ÆÍÚ=ù‹?`½ÀwwXn?sžnfÖr?'>xê=?"椔he?î_XubÓ?ôŠ1ðޒ?^@íŸlú¥?i/ãÚ?©qAù?ò¬ö€E?îi®€_ƒ?˜aœœ=ü?€lŠF²Be?u 63Ç?¥Iý3£Ä¶?™>F«˜Ç"AGN4FGL J1428.9+5406¿Ï¾mt³ÂK@LÑM"‰aÀ:¾VCæÀ<Ÿñpv‹@ЉÒ|97@èÃm¨z?Ço<8j¦?¿ƒb¯È°?ôOÆl`{@¶¥ÇzS¿Î~¨<¿3¿êm-]0]¿âP÷†®¿ì¹›Aº_¿ÝäYüu±Þ¿ïÿ-r)HAGNfsrqS4 1427+543?ïò³nVõ°?S«*ß[¿?6k;c¤÷«?1õaœ§ð?TþT¦?Û:?P­ÂG?ïØðÃ2Uy?mŽéOIG?A°'X{<o?IäOH[D:?qQŽ</Ð?iã"TOô?ï|oý"ê?†~s­´Ÿ(?bÚ#­pDm?næÙ%¾0?Œ-w¹HVH?"ÈE9½]?ïàÖ¿e†?KH	|²ã1?HÂ,e+e?//¾çí#‰?høµç¸ m?I˜&ÙìC?ïÙøCóõ±?oeãæ2?K®Ï´"•?G¦ù0/?oä£Ã?lÛ>ék‡A?ïcœÿÌ÷?†¿jÂP¬?VD@k
l?^‡9Ž¤Åˆ?^«Ÿ°©?…sÂe,äì?ï
N(	¼ö?J-nÏËÃ?l':u·/?s.{Û?›$QúJi?Ž¨£Ô"Fä?ï˜6ʎÑa?pÇ»'°?aóËÒn|Ö?QÀc>!½?…uZjÇ®‡?o	ºº`Ä}AGN4FGL J1429.8-3058?ï͍eiøR@;Voç¨mÀ;&Ìÿ!³¯À<'ütðm@ ´1ð'ú™?ÿ¬ÇÔ?ˆ?ÌZ.õ‹ÝÄ?ªŸFàAÒ;?äþraFl?þ(V†?u?ï]}>o&~?ìl]¡Eà_¿èç£è§ô¦¿ØUÃ`½Z¿ì¦€‡ÏÃ?ßOµIùHVAGNbcuNVSS J142940-310013?ïƒüº{?"e¸ÿV?bª8¡ÔË?Wfv'ã‡?›L¾Oäø?"Ú@ítÑÓ?ïYôØÚw/?òNÁ£Ñ?s´SF˜O?y«î[–í?¨ ²?ˆ4×øád?î'ÉœITæ?–wh`Ih?uw©ß&á?vVØèµS?¤$qßsè?•3fnOè?îÜÔ²¹?Šš5&ћ¬?'ñ}ô1ª?y<"øIy-?¤¹؜Fš?†ŽJ")?î	@÷Ó?§n™ìžÐð?o5o½A?cKSكÛ?­{æßÿ?¦û0}ê?îG³MIßÈ?¬Wò½ô®?†Xf
	¿?"W‡–ÛÐÖ?¥îÊÒ»h?¥º†Ï '?íbš§¿)Õ?¢ìgǃ?{ùÌÝ?w©­ˆÅÔ?³+š~ð¿?¡ö*Αœ@?ê×¢›B]•?£ýݼžD?¦²¹¥Mð?–¦¢ 
×þ?½éŽRØXá?¡R§xêAGN4FGL J1431.1-3120?ïÿ6tŽÐÆ@:ßlœ
"À9ÛÖ¶Zš€À</OC427@òˆQ¬y?þ̦6`^?¹"y™I?³¼f"HÕ1?ûº"ԗœ@-îdÍ	?ïÇ P ¿æçÌÍ£Œb¿ÑíÔñhŽ¿àŸß|&í¿Ý¡l å}É¿Üå6%+ÁAGNbllPKS 1428-311?ïùâîæìÍ?BOp3p?"\V…C~?ÕúUQ?CÝ.ŸŒ#ˆ?A	¯7'?ïèù¢Ü'?gâJ
Û¾<?7)œó—½F?F¶ÿcñÝ?d!Êí±ï0?d*¦®•S3?ï¢8Ÿ·HŠ?€öÎþ&HV?cˆtn?
p?tL6Í?'»lNß?z{:ž5"w?ïÞilÖ#?P«} W?8s@5í
?jPn"gÔ?nˆ0ÇèFY?O=Öo'=U?ïùžµôTa?=PÓûæ]?(Vå/?#:P;U†‡?Coo'ã?8EnA"?﷈ñ'äU?€¢õø°¤?L©®Òº?ZøJÔå?€S2]D†œ?~<'+âï?ïk˜Ž'?…oߖ;ß?fÍßîÓâà?r_èN"±¤?fg–{ÒÀ?ƒMiD†$™?ï£ÈV<ð?lýÉcõ"Š?N˜öL‰È?8ŽdWӆ'?…Q~'š5?l–"ƒ¢ÅAGN4FGL J1432.2+5051¿ï`Ù²õqm@MÄ}¡ìNrÀ;Œ¡c'wÀ<ÓGºÇè@âõLÈ°ˆ@Ú6º§0[?Á³±]Z¤?Šo*%sÇ?ÈÔÁÔiy@
qŽ¯/Øá¿ëÿ˒:)Ç¿ßii:¬#_¿å÷·ÒiſݑÅÚ뛿é"±œ]™¿×œªZ±ý>AGNbcuNVSS J143217+505603?ï󓨓Ým?KÞ;Ê}ª¯?=.ŒIí¼^?0 ¹"¬??QÅɶâ?FúUï<Ì?ïÞÝ®ÏêA?o‹¶Gü ?9‰Æ²Ñêy?EXvӔ™Š?mñ™Çl\?l{'ä•;?索6Të?|8ÜP´‰›?W•ÿ9ë5ÿ?]™Æi"Ì?ƒ¢¿"ÌF'?z÷x>4ò?ïæ0I…d?Iހz9u?D³èömÓ|?'Y«»mˆ?d¢¼dÁÿ?H"³K¿~:?ïÚ©D?l_¾m—À?T¤{âÞãÏ?MFwÓâõ?k}&í
Í?f½'"2s?ï…'Pq?'é	T£¬~?QbêÄÑ?ZÖÎÖ)ÔM?Œš/Â4?'=bQ§ê?ï2Ó_k¨ù?P5nB?d¸\­Ê?hò'RW×?—ˆ{[g?Œ;Á£Ù ‰?ï¬õ!]Pq?iàqß\A­?`CÆP¡K?Kn1Uj'T?€±Æ*Zü?h[¬A	àAGN4FGL J1432.8+7648¿ëÏu!{a@Co8q`•lÀ:ôÞü*ˆÀ<Äh-ƒ@
Ž+§M·@Œð=ë?ÀA°¹ñ¨Ï¿±¸©)Y•ž?ðôu£KÜ?øS¸8ìË?Òpõ5¡¢}¿ä‡£'¦ô¿åJù"–,þ¿æ°ÔéÑÀR¿ÍÇNH7|C¿ïûܟ¨§TAGNbcuGALEXASC J143211.35+764355.6?ï»ÚÂXÖ?zm^bkñõ?[2àëNUk?Qv'Œt?{¦ÚQrý?xKáào=é?ïX¿Ù8.ß?Ž¡Óõ
?s/wõ4–?x6ÓUñÜÎ?!¨1è?†'K.Œe?ï$¼FÔ?†ˆ§}ɐ?u›z_Ž¦7?vºÏ'ƒ‰?–Ÿj9ÿ?ƒ9zȳ?ï*œ9˜8W?x»Pæ×-?~'"6âÎï?i
•V¡Fì?"""ÀÌi?t)T®tDe?ïLQ+¹
Ë?9:· ?u±Â-­$u?p&N·)??'	j²?‰vjl9Ìñ?î9¹rZ™?¥{wÉÔä?‡5c£¹99?'RIsÈkí?¦ ûƒ[¤? ŸR&¿?îb²]›ø«?"?Êw0XÐ?ƒKL@Š´?]…Ài/?¤ñ‡S\M¨?Ž"鞳˜?ìü՘ÖÚ?—©ßœd"Š?šã}ŸZQD?Œb
…1??±f™ê†Íã?"nÎóKDUAGN4FGL J1433.0-1801?ÊTU¤™ŸE@CIM½øôsÀ::DZ°èÀ<~ó%&*@u2¹e¼È@(ãúü?ÂÆñÁxÛ´?Õ}BuñI@	'^VÍl/@ù
ÒÁÙ?×Ýê¬\¿Ó(ؼD>s¿éS³`À	E¿êR·ÈXÉÆ¿èÕÙ ð¥ð¿ïÿì»"AGNfsrqPKS 1430-178?ïq9ېVq?‰Cv#'4h?zv¡SÒº?sEËìž–?†v8nðôU?ƒú*Êú$Í?ïÙº'Ù(?qB©="˜Õ?G›ãFýÅd?U{ |>¾?p‹&e¢¢©?l/VXËùá?ì\¯´RÐ?¦³X&?¤¬hõª%?™c͝~Â?²ÄN—ˆ_o?¢—9eMøá?ï͹g"?TU7õy¼?U	`$ý–;?8HlbBzO?sá%dâ"y?Qn?åÿfé?ïVcÎÓڀ?Œ*uZ±7¬?~wå(á
2?wU1EÂ_?‹+¼È%|?…Ò?añŠè?ï|¥í•?ÃIŒÔ
?_c2èÕ(?hæ'yZ?Œôîå«+?Œ ]23?ë³Rš×‡;?ª+ÝïØí!?¨÷ÅRgÓd?œÆ?åª0™?µéˆÇªt?¥¦döR@å?ïh½5ÄÍ?v§"^a©?p)ƒ+ú÷Ü?[*J¹0Ú?æ#pˆÙ?sn)Up>;AGN4FGL J1433.7-7304¿è*1Q†°^À'`†`ÔÀ;°¥R4€:À<Ï0é¬×@#1©kž´Œ?ڐþ?‹†1?ãќ	¶b'?ïù½€Ô{Ã@®ì?þÛ3,}6?ëå² ùõ¥¿îޜ¾H'¿ïԋÝï4?ïŒv›gÏó¿Ç{ô'žUk¿Ï¡&Á4éAGNbcu1RXS J143343.2-730433?ì˜ɾÇÉ?¶n›yç¤I?pg‰í I¸?j¼"ùq—?º9`›\?¶8|•æ?çÁT˜!Ž4?ÍQPŒÐr?ˆé"Í"Ø?—CøZø§¥?Ïx?̐WŽå¿?ìkÙöè…?¦ˆÔi=?‹À½1ê¬Þ?‰ÝwÆ´O•?¹)¢:À?¥^´$,l?ë*Œñj'?°xv'à?oªqŽ{Ãò?}ODæ€ÔY?Ã<¬ø"®?°6`Ô?껺'ê¢î?Â%€(j"?ŠøYç~´#?•¢Wè¦|?ÃaUo•‡?ÁWL¼Šú?áÿŸ4?Ò¶I"È?"umW€ÌB?§ê÷Ñ¥}?Úº‹ðAN²?ÒyL<n›>?êZû?73¯?¯Á¤¥'I"?'	ÍK\Q?%*ýq¿½?ÄqQÉBËú?¯°	›ÕÌ?å%&;d?Äl¸ÿª4?}fú'_
?Š‹€Š1?ÕÌ—¨J?Ä'S^ªbóAGN4FGL J1434.2+4204?îWø—€å™@PC¿rq7À:GÞ
ò}À<¡("V@éùK/ÿ@—!œ1ú?¶ÍàsØ(?‹¨Mˆì?ш¾ÀoœE@_ˆü"d¿áÀç@Áf<¿æÉì}l<i¿æS.°ís6¿ãFñ÷(Àé¿ê''ÿNTL¿ïÿÉ¿&FAGNfsrq3FGL J1434.1+4203B3 1432+422?ïâ>"ø?bœ¿u?Uî°q×C­?M2Ú°S²?bʔS€¥î?Ze;iE½q?ïÒYxÛù?|ÇgfÔ?J^^Ê46?TÃéR@I?s­QÜUQ?z}²'Ù?E*p?{žSOL?d§ú/.Šc?n<r7…k?ƒïp>ðn?u•f	z¦?ï×¹E"?SÝ°_"Ñ?dôãH?KXï…Ì?cR)‹É08?Em0)À?ï­,Ôz¿?yHê/8?p"ò#˜"?c=V2 Àò?yNrù§Â?s7¿mÁ_?ïn©›;ҋ?•¤XsæTÿ?\Ænᢃ`?iŸE	/bÉ?^e®3V?""
S@=	?ï8Kc*Ǫ?†Àd½!'©?qžMãٝÜ?tMg^{é?")ÌE?"d÷9~š?Ú	æ?rŸòt·B?®Ìøò?iYw+aØå?yå'$VÒB?ceõ…"5AGN4FGL J1434.7+1950¿é´.Eì&@PR2LƒfQÀ8· ·›`À;¯–ú'è}@ْÔ-"8@)(v>K?£ß¾þQþ?ÁŒšBç±@´[זT@Â*­¨š>¿Å²@Äì-»¿ßÃp,¸Å¯¿äì|•|Ôg¿å1" Ü.¿è`½¨"¿ë‹q¾‰=AGNfsrq3FGL J1434.6+1951OQ 253?ïãK£[S'?\ÿÖî$H?TšÅ	%?ð?Pmr®[?bfùúþq‰?Tgx6æs?ïÆ!'*B?yBÏ£6?Tò0¶å…"?j[bnó?w²¤ûs
Ÿ?qZ!Z'ô¨?ï†æ"iÌ?S8ÑFž?|¸üœŽ‹?…K)ôñ?ÓºFÌ8ñ?€ÒÂ/;•?ïʍWÊu?aDa!Ž¶3?ZQâóxÁ?D\="³?t]ÀµGW?]Ê
eP_<?ïÁ‹u¿tË?t®eiÐ?b€ÏäPlj?dD©£?uùÝ?Kpr?l¯xJ3ëÃ?ïo­óvbf?Yê84Ó0?d{þ½X8?süvÌMÀ?Žõƒb;,©?Š"‹ƒC{\?ïhUåm`3?Ž3t­™.N?}"øeƒ?…a'e›F_?‡!©ÕHi?"˧ƒ8?ïRƒ¬-¬?',!%ï?u½zÆ,,?d''ÌÁ?@+ÐN®?€@ïÙ̍AGN4FGL J1434.8+6640?Ì1ùöZ†@G°K±¯:À;1ñÛzºÀ<äŸê²ð@!gŠS*Ÿf?ù~N"ÈQ=?ÄMoßáÒm?½£Ž¡)A(?ù`¿'țæ@=qá¿ï'ëk¿é,%Â!ù?ïý7cCœ7¿Îëð¾ïi…¿ÞšÜDŽû0¿Ðï¯OäCâAGNbll3FGL J1434.6+66401RXS J143442.0+664031?ïØð×"Þ?†ˆ€¥Sw|?B&LG/ý\?Wr@ip"º?qC'tɍ¡?"›B…€?ï¾ÙãœÙ%?g"†Õw6?Q'º7،.?[°g=à6?|IŽÿ¢c?z"›ì=¬?ïi`O\Dá?WҜëî±?\Þ"~'Õ?U<ÀLü%?'h2OzÀ?«j/&g?ïXO)ïú?r0e뚬å?`õOBøi?Qg–RF?'ßÌ,3§²?qÁƒ‰ ?ïʲ–&?rá¿Ïk"?G€+›ìøÝ?C°iŽƒ9??x!`¢?qçjPäp™?ï&/VQ<Ö?šÌwH~!ƒ?e*!;	þs?tµl"N?˜"Ñö…m?˜Šÿ.7?îíXV	?Œ	Ä
É]?a1s:]?Pg¤ÝFü? ãD	N›?‹•n*™Ë\?îZOIòÅã?<¬š'_?q5 tøÎ?kÁ-a?¨4WP—ô³?»Æ*¡AGN4FGL J1435.3+7120?в
õ6Ã@E¼®§GØÀ<*¡/"À=˜w:Ê@:ë&ÿô?ÿ ´%6n?Ö¬æ0x?æH"Lx~—@~*šÞ=8@:¾÷!4¿ïÿúÁҝÇ?ð¿×V'þõ¾Þ¿á(ۋ¬q
¿ïþš9҉¥¿¡NöºKAGNbcuNVSS J143518+711818?ìötǹMÐ?¼zŠJFJ<?¯eM5a?·¨A"#^?¡3fƒÉvø?¦'s­
ú?í"ÁC4eÁ?ªåxí|O?¢{¤íùå? –ÍCa ü?¥8FÝþÜ?UqðÝ?è[ít•±¶?±°î:ìÌ-?¹ƒÙ°½#?§ëܖ=?ÁÎ]¬¿¢S?¬U±0ž?î*b ™ò?‰Æ5­¥?§ÑÃÌù?†ÂuÓ8C5?†#$"×f?o·²9õ®f?ìTgà'â6?½52QOÃ?³O¦åRAÑ?·…Oâ«?¤42ÝXþ?©çSÔÆôÏ?éûo¿wñö?ºX&ÔøaÈ?µÇ(ú[aŒ?²9Ñî*ݨ?º]Y
Ð>?­З€¼]?æV-
]?µ$Ìd³c
?¾¶èÊYU?­8»¤¯—ö?ȇ3n 	?²átïþ?ëŠÝ¿–áâ?£ÊÙWŸ¤?ºÝZ?¡•Y¬Cª?¡˜)dÓ?Žiì)tÉAGN4FGL J1435.5+2021¿è̽öù¤¥@PRžì¿±[À:"F}'ÒÖÀ<]	ÆR_@!S«Èp?ÿ0L齞\?Ìã^ÊÙ?Ïqßy¹Õ@hÞ£Žåá@—Ò- ¿ï]ÔA5Tv?ïݤ@;¯Y¿æV>@¢Â¿ÈðšÝ;"æ¿è;`gÊ¿ðAGNbll3FGL J1435.2+2023TXS 1433+205?ïqÙÍCô?…4ëZ†¨3?põ_ÒF^?d÷×?©ý'?‹°NÚ/ë?ºÎ~Bó?ï5Å·YÈô?–"Èp†K?
&'ÑD?†zNãƒk²?À¶ÓÏ?Œøø=­¤W?í'jZM? ÃòL}?"ò놷?ŽoÉÄ?­Ò¯çn µ?™œ¦>à¿?ë^;óÝC#?•"ËYĽ@?¯¿üøž÷?Ty•?µ."X=°o?ŒûŒ:ÑÜ-?î,Yç@Û+?«˜Â'¸ß?‹h㗊7á?ŠÂϕ•X?¦`(§ÇP?¦>7þÄÈ?í˜ú¸B|&?±ÓŽ£Øs?™O;ì.*Ï?¢é‡ôy»¸?©È¶‡xö/?¥š¿ííä?êc)¾xn?­+Š–~?¨jI?§f?›j I'C?ÀXƤ®dq?¦¿éµFær?æç˜V½?Ö?©µ'•k[?¼¿ùóªå?¤Ñí6?P?Æ¡«5ù6?¡xŸ¥%AGN4FGL J1435.7+6148¿ïËÔužÎÉ@I›ÝÁç–}À;Ÿ{DDÀ<ì'ódK@ÌšY²ú@t` Ò?Ç;XE¼LÍ¿«F&CÐS.?âå7ýO@ª)¤"…?ïéóïP…T¿æxcôœ¯¿éwÙ.Úß¿·ÅC–'¹¿ã}:ÞxEâ¿ïê¶øO1–AGNbcu2MASS J14363365+6149514?ïÕ1!?rãÅ­å>?P^jþéø?Dñ¶wBj?qOâOš¹×?qï^z½>?ï¸ß]PÆ ?}£þU|x?R¯þ²»e/?XO€!̤ ?~äQÂûÉ?{#òFX§Õ?ï#LÛG?¥ÚNþ[^?pÁðÎ÷?tÿÅéræ£?˜KUÊÔþ^?‰Û
ZÆ?ïÊ¡ª<݊?^xü#¨)î?XK‰9åC?Df‡zs'?tœHÁ¹?[×:gnŸ?ﵧý4ž˜?wó¸™n…?]Xˆ¬¥?U×!(Ø/?}ÕЩh«"?uþÚi' ?ïBð±áí?•s¢œÊ?d֖T¾¾?wÿ½|Té?•#!&³v?'TØï½4?îwÆIGî?'í;ƒîõ\?x;¨y8?vŠ¶óË?¥|8,8º~?'wHËp¸A?ï9Õâ?(jþÈÊ?xø áœœ?pÐ+Î{RÑ?'ŸwjtÜÚ?|Bš­3‹
AGN4FGL J1435.9-8348¿Ûƒó]7òÀ5ˆx·¡Â]À9ñ¸'ƒ$ãÀ</R1%;ú@™]f¤S@ë=Ñææ?¼ÄŸ½Ü*I?¶ª›I?øSëõ‡:@,'y@³¤¿Ö.á_+¿æÁIÁ•?¿è½0w—¿âÎý'¿ïö6¾.®¿ïüɟpÉAGNbcuPMN J1433-8340?ïözP†³Á?Aq"å8Î?0î~¨/‰?"—ÃUAÍ?MŸ~£ÕÆ?>1ùklOú?ïåø¾˜,?pEpdþo¥?>x \Œ!j?MP…Ç´Bë?g%äí?kšúTdD?ïÄ(ñ»Ä'?n€9—ï?\\2<
?c—³Lµp©?vԀ?x!?dG©:?ïÔsį?QÜN˜lÝ?Q'-Âßü¾?5V5¿Œ"6?q:'ÓwÑ?OÆã÷7¥?ïïCášþã?Q<…¥Ç~r?@4"³†Ç?2ôü#-?Y]îMži?N3¿b'…?ï°¢ÀglS?Š8¦å‡ƒÂ?QO•õ¯I?lfÃýr|?­]ÂèR?…òúü
–¼?ßlW?sÁÀLü×?dèw2Z?iåÁ•€1?äê'ÄÀ?k'$µSúÍ?ï…ï÷~t?q³´ßåO?jÓٔ"ÿ}?W\ Ýö?‡Ï)¡Î—3?mÊ·ÓOJ¦AGN4FGL J1436.9+2321¿—ßcqLE@Py©?)
»À:y|ßýÀ<Q'N"¢Â@ý1Äs7@‰
5
(?¾)j1¢ˆ?¯ç¸Ëôœ?ëSÛIgR@Ño‹þüJ¿æCŸu¦ ¿ãdc1Ù¿ä}P·
H¿é›K_ú¼t¿Ý'ù\wпïîÊM–ŒAGNfsrq3FGL J1436.8+2322PKS B1434+235?ïÑOqŸU?qÔõî·¶Ä?L¶¦*åyN?BviO?I?sÁªí "?pﲘö?ïÔGªäo¬?s"ƒŸ¨Î?Hž¥ $?QØ~¼šÃ?rÃÖØä
(?pNšàž?ïŠî·O¯?z•jÇr?b"zY3_?c­lá0V?ˆòýdÏud?wåôd¹©?ï´ûAÕ7?`9Iâ±?e¹XìuG¡?Màai´r?z¥²³XZ?YòhLûr[?ï¤6§?~¬šÌKQö?ZæzT?QÌð´_¤õ?ƒ›c?|[>ñ&¦6?ïyˆF'gÆ?Š«ÉÇߨ?ZƒÝ‡—b?cy·¡Ó3?ŽMr¤=–?ˆoLÀZË?îî,mò ï?'g²vWs?r1s9{?mV(Wl`l?®süôT?‹fyQg¶?ï)4½Þ»?€%ïïŒÎY?~ÁÛðgÄÓ?mµ‹Ã½6†?"(ñLD[?y•KWŸ´AGN4FGL J1436.9+5638¿î.öF²…¾@KuâlvÀ9½Ö»cýÀ<\u¼D¿M@†òÍ<‰H?þ©GŒ†Œ?®¶cC‹	?è'u¹?ã#×?íUÙ@	äùÄQ©?íö–•[$¿äEmþ
\z¿ß1uBø";¿Ú›[慱¿Þöú2`¥\¿ÕVÄ-ÁÚAGNbll3FGL J1436.8+5639RBS 1409?ïõÏ[X§r?@'JE÷ú?'¿²!˜³˜?µý°ˆMW?QiS["Ì»?=…Jµaru?ïÙPiW?s»°™µ#0?DùxWS?OoõM°†?pÕL600ÿ?q"ÀdBÞ?ïÂ.jÃå•?jd]8Ɂà?QpåJ9
–?Sa~ŒÛ?¶?zŒ'3q¯?h³°]ä?ï®?Å!?`RÓnŸîd?`'¿¡¾E¾?@Ýjӛ©ö?€KÎցrW?]'³gê(·?ïí°‡œÁí?Qޘñbâ-?7³Æ"°yM?$씎Œ˜¹?^±ÿ©‡e?P>ŸÏÁ$—?ï‡Ú Kœ?ŒXa†{ÜO?Sîï×Q׬?^‹é`¶ãÿ?‹‹ž{£ö?Šd¦^(HV?ï—|yßPC?tÊ¹+ò+?VÔ@œmØw?D#‹h6?‡FYe'ö4?sÖ9‡\?ï Óý˜œ™?~«
T
]¶?vTŽØ4†Þ?^KRDãB?–P\™
?{%GZ*^AGN4FGL J1438.0-3128?ÂW=ØÂh4@:!¦'¶(FÀ:Á"‰cÀ<[¾¤ž@Ö'-ŒÚ@9ö›Ó/½?ЁôRLÔ?֖ê<Ê5Ä@våÚºÌ@	µŽª}AŸ?ﯭ7OË¿Ùùð'Íó¿ç"ré+¨¿æfS¼?¶Ï¿ïç'JïŽ4ÁRÆ!AGNfsrqPKS 1435-311?ïŽS»úþ ?¼·ƒÁ?c·ê]Pð?g3ò£.™u?‡} ÑÝ?‹Ê}¡G?ïn,OFî?ˆê!ìŽ+?s¨wÖlÝö?t¡¦Ð±*Q?Š¥¹'?÷Кƒl»?ï+©ƒ
zÇ?‰a¢ºÞ?{Ò}ª<Œs?xäŸOY»"?"–07éý?"ºá •ø?î½Q€êåÖ?xiV^!?ŠaµcÀ?g
?GÚZb?›%L‰©3+?tVÉA¨C?ï=S
ªHÐ?OY£m)?mbÙ$B—?è¬Ý?"©C(öM¸?F"#@w?î¥Ü7ùÁx?¢Ng|r´?"¿¤—ºÌc?ŒBU%{"? rSX½gq?š5ô"F?î¯rÐ©7?"-±ò‰}u?ZÈ'I?{03"9	e? ²$þ,ºJ?'BÇ¿k?썇C«¯?"Ùƒì™?ŸÏÄnœzP?"Ö1mMp?³ŸÖñ©v?'Ž44×eAGN4FGL J1438.5-4207¿îÝ|a>M1@0w>Õ'åÀ;g˜ûÀ<'œ£9UŒ@ ÷Öå¼]?þYÖÖ;
˜?Í0!ÌX‰?²Êö†M?äâ6kw@z7y>s?îØàkæ(¿ín¯½µƒ¿È¡šïÚîοÝÓÙ{±Ò ¿ãÉ?2Ȫ¿Ø;vBýU¬AGNbcu3FGL J1438.6-4209SUMSS J143836-420705?{֐?ƒî'ÞMôò?BÉÛxÌï?0âBó~öá?‹kÃD#J§?ƒ¾‹çl?î|pT•ê?¨u²öÂ&œ?~ړ*[?€l¹¥d;?¤x7®R'?¦w¬p-ï?ïNÝ/	q³?2¹Dœw?`Y´!ëBE?Oâ<X˜?"#—¨¶j?€˜\‰z?í"âFAéë?‹/-é=?x¯VO±î?ZW¨Ÿ"Dû?±ÕøgiÍw?‹™ªšú–?îÍF ´|/?œ,³¥$
x?QÛïÖc¨?EÓèìc+?¢œ¶z=i?›÷ÊTáÿp?ì¸_<Ì?ºXuâÛ,?‡¼­BqS?mG•Q?·E"7'v¡?¹s'-T<'?QIÒ:?"<¿nð?eþ"4Jîd?Và´K§?¦7!¹¿ýý?'öB"7qV?è´BD7?¥"ãº?¥‰?ŠûTŸ"…^?y4ØÁ¤?Ë~M®¼g?¥ÿmFË­AGN4FGL J1438.6+1205?á"
rZ÷"@N\UÀü´òÀ;jœ×;»˜À<Âk"ÿ@ XÙéëÁ…?ÿª¼¡Ü^:?Ðj"2¯Ö?¤PŸªª¸ü?Õî$5inY@@šÒª?ëæoÖQ°Í¿ãg¾Šêª-¿åØl¨ŸÆÚ¿ÝÊ2ÿÚ
¿âëî›S­ý¿Ë¶^Ì>1"AGNbllRX J1438.3+1204?ïÙ¼OY¸?`¡ŽÒ‹" ?@ÀÁ†¬Ü?0P¬Ýš'©?q	ÀE?_ßwuÛ?ïb[îy?•ï<ÁÚÞç?iÈþîQf®?s
,…@Z‡?{bRÙ·Y?'Þ¦ãüÒ?ïwRíbÄp?yê/£L›ó?^'ó³òK?Cº­Ù³‹?ŽY9Q›®?y¡q˜¶R?ï:²:q¸L?uO¥g'¶c?qD7¢ìo?S&#ü™¤?"X˜Þ¸Ñ{?tÊYS¦Ô?ï©"pÓ$?x˜PUò<«?LsütN	‡?="Ksi‹"?ƒð$<`³"?wº¨u%Ü?î¢Ä¦Ċ?¥Bù•ÂY?sÎۏ8W?"F ceg§?£YÚ;>b?£Ñ^]ח?ïӅ"¿?"‰	å˜0õ?e<mh'?QòáA
Ã?›~ÇÕb?ƒ«È…ìCÛ?ívéè	?"/:;!?…àÀ'Æ‹?t?£o¸tþ?±"8­†ç?"½a˜l
AGN4FGL J1438.9+3710?æγS¡_-@PO6&,ºÀ9+Š¿â¿À<3"l;'@λ³tâ@zŠûq%?§0¹[Uç?»¨w­áz.@q|å-ì¢@AÇn.? ©r]H81¿á¤¢š¿æNS™Û¿ä¿-½R†`¿ëö{A"ÊÓ¿ïÿþˆ0»ŠAGNfsrq3FGL J1438.7+3710B2 1436+37B?ïÖÏÄñ-¢?f}øνM¸?[•®•6­ñ?S`$v5 #?ked_?`Ž0¶²S?ïÏô%™?tOlÍORõ?L›QBJ?Z<Z@>¼°?tä›Õnëö?pDKJ†#?ï'ùs?¼?BÿBћ?s™Z7Ž¡–?x·)e<º?´ö,o².?y]Yû£ò?ïòsßî	*?<zÌb"°?E¸DÕ§?/Í.²Ü¤€?PŒ²í[ð7?3è;–ß~?ï±ô…^µS?x½5j
t?cܱÙÚW?_†
º#î?}dMlýR?tÐB	$?õ?ðjûe?‹'&ÒHß?_",ã&m5?w'ÚàÀ°n?‹­>O¤ü?‡©3•ƒµW?ïObþŸO3?ŠgµdÞùa?yß_¶ÈÎ@?{«dÇÓ²P?7~א9?…UMå;.?ïܞœm£?[ ì0?\y¹žÂ?LÝ*·y'?e%ãCé?R£§Tº6ÞAGN4FGL J1439.3+3932?î°7…äl@PêÈ`V'À9åßÁœ"À<cv­‡@ú—Ý+ê•?ÿ<ÛØÙJŠ?±ÍFšC7¸?"'¬¨{E?áªSÆP±É@¸ï&&?ï"ÞnµÀ¿àç­=»Lr¿Û×!ºdë¿áKs›Ù¿Ú|[Wð¿å§«ÅìAGNbll3FGL J1439.2+3931PG 1437+398?ïå\¢\$³?Y%Úã™u?Bb©jýÕ=?38Rô¾){?f
³?6''?V_ՂÇÓ»?ïÙäÞo>?qf–T›-Ý?D9qúI"t?P
¶þ?V?p†bª¤Õ?m<þ©äÎu?ï°¡š2àl?rŠÒ€Ï?T€Á1?@Ôc{?G^8iY?qüž•yþ?ï°÷<ÉL?`'™/`õŸ?fmÚ86?HÞ/sp	?|MtžSºØ?["pÎÖ?ïË^/,µ¸?l=ÄbAQþ?TcÄ'ªm?G®øÅÅt`?u7÷yùF?hܵgöGf?ïÐ(]'Š?‰Æ›5Œ?Wvš÷t¹Ž?a†ÍXʲ?""nPY?‡Ò'ÀƒÔ'?ïyJ¬v–	?~ÒN¿O"?]©=àè?NÝýÕG?ø-"ÍàH?}§îžZ~?ï>ÔÁZJF?xÿÀöBý'?z8MúãÏ0?b›Ý]•Ì?'—TV)¾|?uŒ[}µ#—AGN4FGL J1439.5-2525?Ë#•Ñü­@?ZäâmHÀ;VìÔªÀ<"1í¸ÕŸ@!¡[YíÝ?ùˆ²¡)±?Ð<`CÃX?ÊH)åV±h?ü‰l«$™?÷˜ùöüv3?áÕT%B|?ït§!A™(?Ìóä餿Í=þhPK¿ÖagäjÎ*¿ã9oÀtzAGNbcuNVSS J143934-252458?ï8B2™I,?—.š—ýT'?d΋!f?jêsvþ7Ì?–]èKTþd?"—oãþó?ïlÊ&¬Î?Œ9neØ.Ò?qb¾ü«'å?x?k¶îzX?Œ 7§ÿ?ƒf݆º¹	?îøtrœk?äëUǛ?}€Í·WÁo?Ný"ž·p?™'>X	¿7?ŠP"D]?ìåú"/Œ?'bÕÖÇß?"Ò	Jø
þ?yý;â?³›­6'¾¤?Ž^`®L¡G?+¨?ŸB¤À>I?s§2™m~?pìŸÒK}?£AFó䦤?œÙŒ)¼Á?îµñ¤¦º?¡8ŽþXñ?'KùCöiq?'¤©Oì'À? 
çi7þ?˜[•Ž-eû?î¸hÖr?˜Š¹¿ÅK{?ˆR#*ªã?‡ÿ+f,§?§ïð¦6Y/?"­Óæ±S?éл3tw?¨0Î:F^?œýòô"?‹{6Ik˜?ÅUƒó¥?§dÆÓ3zHAGN4FGL J1439.7+4958?ïÇÅàä¾@M–ýuâlÀ9±vi騦À<~[òoÅ@ó@7'´z@0«~žk?¯ey"øõÂ?¦&ŒÝ9¬?öa	ÐcZB@¨öæ%ä?ïôÁrüvß¿ã±b]Ã)¶¿åªbÆ[¿åÕò—Ÿï¿ÝnÊ£|ÇQ¿ïÿ–]ÏéãAGNbll3FGL J1440.1+4955GB6 J1439+4958?ïێÄS‡?£#…ÀC³{?2àÃfÅhç?$¾ƒÔ­>?q
'"b¶??£$e6õç?ïڒL6ß?nAQg$t?Eõ¦†­?M×RýaYA?oðJDžÈ?i=Z*MC?︴ép
n?p¾ÁI42?XÊŒÞË?X_v§ah?}s…–ò?nG®ÃJ?ïå"»é?KJbUú:¹?XWdÔ¯?>¢ȩ́U÷?]{"~2o?AèëÖ£Ö?ïÚ¯_R?d­=¥þÞ?CÝójžÕ?;5ù#c?p|êe™?bÿa1æ²r?ñÑò"?ˆ½Í'©ò>?V~4!¾k^?bTÐ0–`(?‰'<÷%g£?†!?¨§ù?ˆÌº?zPõ³BYŽ?cRžÛ'U_?cúõÂuï
?ˆ©5Ûé|.?vª×Ð#'ÿ?ﶜl{?h~Ô€Ò ¿?q@øƒ·í†?^ ûÍB¶?s±¹B Ì×?_2ÒRWA¯AGN4FGL J1439.9-3953¿áýƒø·P(@2_ûz_A¯À:WKtr˜¤À<Eˆt®'Æ@ ¯ÔH@ïÏÃøõ?ºB3@Êž¿ ±ÇÈªÿ?箨—›@ûÐE}8?ïþ*"y¿¼WÆåW¿éiæM§RÀ¿ÓýãÆ
–¿áWpßçÞ¿Ü -1'r"AGNbll3FGL J1440.0-39551RXS J143949.8-395524?ï¡ÝzÄí/?²Ck²ÿ?T¬?¦˜Œ}?Wj·FZ«?"óYñ¢•?|AÈušÏ?ïÑ|՜1Ø?s' '-?GN˜Rz
ƒ?Pw·g¤ñ?tWÂ+ډ"?pCTYƵO?ïkË*¾Î?""Îӈ	?cýIŸäÀ?fF·¢(Ác?"Úø	Ž?ƒ– ¾ë{w?ïd6wz#Ì?hÇݐp¦]?h¸ïëçe?HU…«<?b@#?h+Áôßiø?ïa\2IÃ?ŠÂC@xii?dd*_¦¹?a4Àæa4?'Gøí0'b?ˆo
a¹ï«?ï€ÿºÆ?ŠSCŒZÂ?Y¾
ˋ³@?fG¹÷êÈ?ŒÆ>îFQð?‡Èã¢ëì'?îÛØb÷?'ÜŒà.·?p/X›j.¾?rQ¹È']? <ŽÊµOÀ?'5õ˸V?î—:]¿?†nsËà°Þ?"gó'm´?k‡÷u4çì?©|"$h)?…Y¹ïJ\7AGN4FGL J1440.0-2343?îµP <²@@elaR*oÀ:!…óÊg˜À<OþR€ÖT@vq·þ4@†ý»'"?¶÷*nh"g¿œ[¶ùÀ–?å®:ÀÆ.M@´t'ˆÛÜ?ïõi~sÎY¿éF
¹üæ¿á?ž¡cê¿ÙBÔ{lÝÏ¿ä¯ÄH™ÌÅ¿š"!J'–AGNbllPMN J1439-2341?ïâÑçòK?X'ê'¡¤»?CѹN«?15TE7|?i-yÞñN?V½¬!÷@¨?ïÜ&IÇí?nÑ"áC3×?BL¬2";u?LÝÜ÷g‰ë?oF̵«>!?iÔÿT–%¸?ïœîr[^˜?vdAfl€?Y0xbi´?^_diäº?…žTqúÌÃ?t¦Ð"ì$?ï£hÈ@v?`¼ Vºˆe?b'Ô 3o?@öƒÌ–Oê?'œFiŸ?^žãÛ¬Î?ïÃM"lêö?pui¼{?R¿¶Åi£'?CLpèTô?y©H– X/?n²Áwà?SÊ
-?†g3ə?R''Œ?]ÝmÃ?‡:¹/#>?"|Mu­?ï,Ý*Šd•?ˆ€€¯B^?a.CâÊ?W¼ˆöè-?˜>'Rvœ?‡ê0}(þ?îñŸ#¾˜y?}}5 ¦?y҈èå8×?`ðjj
Ü(?›WyRk ¤?zê÷AGN4FGL J1440.0-1530?Ĩ!&–AË@CïìÃã?À9"卍óÀ;ß>>)0{@œ%"¤DÃ@½´'l¤?µ ªDŒ¡ä?–è>€¡Ú?ä&áìÂ@@beOåñ?ïöÒYԇ¬¿ä³5è³2¿åŽF´ð75¿ãkã]²ã˜¿Ýg5c'¿åò#žj¹²AGNbll3FGL J1440.2-1538PKS 1437-153?ïôfʁx?D])±ÒΓ?1K+¬x¢o?"ÀÈ( Ts?Rß¡`™e?AÜ»rßj?ïç!Nõ?i7)?ô÷‹?6lî€÷èw?C)XÿñÚ?fZõ\Ì~?eÀÌ[1WÓ?}‡Gæ?y5w¾ 	Q?bá]º²¤F?gD"¹¨Ë?"˜	+	ßv?v?ò¤ÆË
?ïÕö	QÊ?Tªçv{šF?>C1õoÕ? ÏeqóÅ?s ¿»[Ô?Tޒэ)?ïð~†~ðÝ?N´«rl?8Öbz,¸?+U$Zm¤?XÍZäď?J¼kXÑô?直=Ýlh?ˆ¶õdy/?Gm
ín?U
6ÒàÇ?ƒßy¯žˆ?ˆ…=˜O?ïPÉÿñoø?‡¸øún*?r¸Ø>C?yÄ4œB­?'8‰óÚ
ð?'3›5šX?ïƒA?)Os?tEýëFÃ0?W°jíŠ?B«ˆ`ìC²?Œ9¢õ5Ü?sÈñ¶')AGN4FGL J1440.6-3846?£Û
ãZ'O@3S™åóíÀ9›Ò<xVSÀ;ýF[.$@!ˆjüx6?úËP`j£ã?¶>iN?S?¨H‡-[X?óÏ
D& ~@P7~òNg?ïÿîBt!¿è•Óa'¿à—«öÐ+¿Ï 	cr–¿Ö;'}E¥ü¿ÐŸ[DÊ4lAGNbll3FGL J1440.4-38451RXS J144037.4-384658?î:Á³zQ'?¯f'ö¶?aáåå®å@?WÒe
.¬?«5ÆmY—?¯-ïÉÉY?ï[EVSý6?'μ]‹Bá?oÑ6çdR?udC÷P®ï?.U|)?êqß|Ž?íD1Ø}Û?¡DÓ™Ø?Š+ՀV{?€ùH²Ÿš¨?³­1 zÎ? º¹¦‰©þ?ì‰Ù4å?
Ï:0?Šç%ʇ%¸?j¶u]Õ<@?¸TQŸ¯Z?5-D—ð³?욡¨ Œl?´.m–½c|?t¢›UóZã?má}Õä
´?¹àÉ_3±?³ÝË>˜œ8?î#M·eSä?«Ô·ùgEÆ?"`wŽð?ŒÎz"»(Ñ?¨³#«Ç<Â?¨˜û¿½£?ë^o"2ë÷?ª**Ý	—?†Ï¶ñu!
?'…lm;ï§?ÁH	ÒR?©dMȺã?çGzBfV÷?¦#ÄvÚ*m? Qœå/m?‡ù}Š
mM?ÎۏÒEˆ?¥ëHç9/ƒAGN4FGL J1440.9+0609?ã;‹úÓ@LJ@c^JÀ9¦K»À5À;ÿˆ}£–@ÆK‰Á4h@uv'[¸?¹XÙµé[y?®ê£§dˆ?ñnkÝËù@
'?úTz?í=b.$¿äõϏõ«é¿á̀v²å¿àùÊÇ9¿án"áÉ´¿ân@$ˆKAGNbll3FGL J1440.9+0610PMN J1440+0610?ïô¿9]¼??¢r±Œ?0ðl—Ê?"‹ï×"Å?REm~ÒÓ«?<$p0b–??ïÎÌ&'C˜?uZ#±cÑh?JxÊéTYw?S^VïpPÎ?uJÓ\	Ën?rHnÒWº?ﻹ£
—Å?j+}P…A?TmÅ÷4Æ,??ïåUzî?}½DCõ?h?†(‡`?ï$Ð:PÄû?rmë:	2?vÕ¶P?¥¶?S<É»£ï?•°‹ û>?q¥ŒÈý?ïíÁYښs?N+åÑŒ1?@2Ší£Ý0?-»)öç}H?\ddís?JX?éûÄ?ïbU9?"Ì6÷À?`AåÒ$?g­Ïøû{?'­P.¾?'­æ¹?ï"¡a?vcj®?_hW+YÑ?\m¢þnÆ·?‡Uʶâe?soD)-¶?풁ˆ€5?ýIUañ?)ô½y5?rÒû»N×s?®Âí"s@–?E÷DÀZkAGN4FGL J1441.6-1522?äi.Uº@CäU•:À:M0o3"'À;ßr)Zl@&+Í@ð¶ß$¾%?ÈUÛ~ÁQ?ÁªQ¢µ?øñzç&ë&@
¾Ûc9¿ës­ÁnË?ïýž%ðT'¿èš[@BH¿åªª˜Å^D¿àCnI‰¶Î¿ïÿÿÊPËAGNfsrq1FGL J1441.7-1538PMN J1441-1523?ïågœá•?`ÖÚÃ^§¿?A"Ÿ±©žò?9ëÏL©?f3{-ûíH?_>9jꍈ?ïÖiŒ>Dè?p_÷?qÄæ?G¼aP"I?NoJ™zU?qÓ­¬kp?k×–jŽ?îˆÖ*™†¤?–+έ%&P?za'ÞÍ'?~ž*Äå?¤&{"y¯–?"¡9›¡?ï*Ÿ³uI?rwìǯ˜?q8ͬ
?TÔ=¶ò(}?–Y¦½ÃØ?qw²÷^$ß?ïÔW
€?gtæÜknð?SJhG&Ü?KWì4n,^?qÚFš/¢?eÏHéÈ?ï'9¦>î}?‡ºÔ,¥-?[Ö¯S‡?a¿âÎÌ?‹öÀ³öq?…S
ÑÛ£?í8¹Jö¹?£)tZªLn?‰ƒy­Òý?†¦7"'û?³	Æs'8?¡tb[Žà?íÀ´žÞ'?Ží©ñh~?…ñc Ù
?tG˜e9é?®x]^ÕÎS?Œ¸]ëGÖAGN4FGL J1441.7+1836?ʹ4‡¤­'@O¢ Ç`À:€œߢ'À<}šYù@REP—@zŘûå?¿dqēm[?°:ŸŸíò?ëæ±Oí@žÍØ¯¿êéôæÇJ¿ÐõùìÀˆ¿Æ4A{†¿ä¾âÿ>9!¿àÙ O–@I¿ÛÅu€	ЎAGNbcuNVSS J144143+183706?ïÖgZ­³?b'ÞðS£5?K?"IòF?8}×/Þ?qdna®?`¹ŒFÖnX?ïÔ*
É?r4©µìB?HÀ~XÓ·?Pˆj†0?rÙÛ=1?nÛ>ÇD±?¸ÇîR?vòYTT?aƒøFôî?bÖùŸR?‡Òp¿tŽa?sˆµ±SOØ?ïco³c'?c´-‹د?fC[2÷?JJ+@õ
?‡bºVÊß?c
†Ây§)?ï¯uWëq?qíü=î?[`WâYò?Iìiè+?€¶¾•Áæœ?o€7ÝaÑs?ïx€
›7î?Œ2"/ýð?YFg‹\?a‹"òZ]i?Ž¼Ó×ïDæ?‰û%!cK?ï(®|wY?"áS‹{i?j»;þO{?f'o"ª&h?—'Èõ×n?'ÔÁCB.?î͏‰Ù?ƒƒéyß?z#…þ œ%?e®[3±ƒ?ŸÅ,tœô?'2ò)(qAGN4FGL J1442.0+4348¿±ŽÛÓåj´@O"úÖËSÀ:x˲À<¯Ä
†k¿@J,\\×?ÿzΝ‡dä?À"¡²í©?µ2»"?÷™WÚ²h@"(¶ØnÁ?î钀J¾¿Þƒº¿Ùõ)¿â!Êö2÷¤¿Ùk*ñER¿âPŠ\ô¿ïÿÂÞ6œAGNbll3FGL J1442.0+4348SDSS J144207.15+434836.6?ïÞõ·ãÂÄ?^ÿR¡?P¤y€þö?As†Ò‰j?h¸€Vôy?X˅ܙº¤?ïÔè?¢Šâ?uW]Ñõ?Ie€5Q'W?Sù㣁c"?r_0&5aG?q—Oo°cI?ï­)öÀÞy?rl=õgÎV?Wq¤sl}:?^†ëŠÑÕ?ÇMÆÚ1÷?pW½n?ï'ÁŠñ­y?a4ë¢1?t–Ë£tì>?Pãƒ
Œ=º?7kªß™?[š±CœÉb?ïÆIØçi?jÞ+{ý$?]­›½‹ëI?QÝ̯Â?uo¬žv¨Ÿ?eFþk
$?ïwß-*8@?ŒonƒÞtÕ?\;/³û†?ec½‹Ÿ?Ž€Ô$$º"?‰ŠŠ[XÙE?ïmĆœ?~mÞÆB›»?b'¸'¼™?\¯ïû_?…#<†s?|…³I%à?îßíÐÊ՞?}™úÚª›?‰Œ¡tÀ'x?lô•2À"L?—;õ*=?wg2'"AAGN4FGL J1442.2+0622¿‰ãoÈwf@L>@(äüÀ:_Ê?SÒæÀ;̒Ü6¯@q§£áò@"†ŸÁÑÇ?ÆXã["‹?ÔjÛöÀf@Ž†ƒ<`@vå¿â€)«|ñ¿Ð%?•í¿è˜b'+=ñ¿æô¥žµ@¿ïÿå}ó Ì?íýݱ žÜAGNbcuSDSS J144212.23+062526.1?ïÃ^àœH²?x¼8o{¡?l÷Ӄ²?iõ¥"ñƒF?o©Kࠋž?m–LŸg`?ï
mÓ[öæ?¦E/ªª?‡¯àRǕY? ¿©ñÍÛ?'zUlÕ&Ÿ?'šFòëŠ÷?ì	†àjŸ—?§g÷ÎÍ?¡ƒîδ–f?"²Î¼«©?¶ñѓ*ö–?£ÛÙaÕ?ª—±?ˆ?´€7¹N?ƒGqkv?m. 6ùµ? VÃxh±?"ùûǸ?ÆM?ƒÌÎæ/²?|'j¶Ú؋?y
ô´Í£?w–20O»A?u𦜽Š—?í°ûÈ/P?´mÚ^ÔÎX?—ùCÉ™y?¤·—œÄeX?¨ó¡œÏ,n?©Ä´8LÜ?êŸð1š›'?¬oMóG¦?§}}{£1?—ßçÂؓf?¿w?´mQß?¨€4:;²€?êžnG—?¬ü®ìÛî¥?¨dL?OŸp?—"¸ÈÙ¯&?Áœs7IH?¨û=ã
\íAGN4FGL J1442.6-4623¿Â;{8…ƒ@(•¶^Ì>2À:Žö¨hiÀ<-_²@ sZwÅ´U?ÿȺiú?¸`u¡æv?"¾¬Åè¤f?܏Û_Œ­x@û-+û¿åՔ«W?ïúhai¿¼…
ìB3¿Þ<ǼAº5¿ã(qGпÜk:¡±SAGNbllSUMSS J144236-462302?ïµdj°…?u›¿jäÒ^?Q|<(
?AþÇyæ"¢?€w]Økó?t¬žKµ?ïÅ^IózG?†A#7g ?MæòLFà?\7ЎfÍL?y"ü¶œL8?"±š*Yä?ït6æs?£›®ý?d‡2usc?k^_Cµ†?ÐyÒd…?z9¹añn»?ïRxÑߍ?otÖ³6>?pN
¾]?Q™v‰vB?'d‰ªSÊ?k¨;yyýÁ?ïcoØnÛD?Š©Mæ?h¢Ÿì]Ѕ?b¾mœ7D?}°ñ)A{?ˆû&ï†tÊ?ï^^-ô?•¾‰Šz9N?`܌ŒÛ?qU=˜ÿ ?'#­g(o?",Òpû•¸?îíþo[?Ž"š}§ó?n¬9ú¨\?pòì\ç7?žj·SÊʗ?ŒIW‡²X±?îzãftÜ©?†ÁWþ¸û?Û9Ð?k‡H9âË?£ÛN¾c?".¦™ãØAGN4FGL J1442.7+1200¿Ý>dÈ4?U@MëöÂiœ|À9èóɐØ*À<1<°Švç@ €&˜ðý?úÏÀÒÆÓ?¸Äßîg§.?¼'‰¡m½7@?¹£ûk@ÜíUÔ¿ï¶PÕÛi?ìyK!K¿Û±EC_¿ÁwkFud¿âï6ÀÁ&¿Ù¤4'NùbAGNbll3FGL J1442.8+12001ES 1440+122?ïà	V¯¨é?_£î«E×?BHeã© í?1°.øÂüù?kdÈÍC?]ÈøQïÜ?ï·y~q'?|Í1dbë?Z¬y'ë]?c¾°Ir\?}˜<ãQª?v>·±–À=?ï‹UÄ,À'?xŠ:³6Ç?a°ó­Ø/?c0`­Û>+?ˆä"µÔ¼?tsš×QÕ?Xž¼?{ëRÔ C»?‰Þˆ×—‡?hJä	<ZG? HI$I&?wÀ°û?ïǾZ¸Q?s«–ý,ž?QGÄ×äA®?D`Ngç?wÎá¾»*þ?r‹?ŸäG¤?ï5Ü ãáx?"a=õ"q?m…]¶¸8?s†v"i?•"Ð&Õt?'ùøä^¸?﵃s×,?‡Š"Ãöø5?lžB¦è¿v?gvˆ»¼3?š‡AK{‰?…¨ØŸëw›?ìÍ ¦¼?"ñ5œJø?›³ ä@?'Ñúî"#î?²«"'—Ï?'A"0¡ÁAGN4FGL J1443.1+5201¿ê¡QFÍ!@L¾Ç¸Õ¦À;X"%"À<ä@¨f»÷@È,å'?ÿ,^YQ«?Çw*Cuu£?ÀåOe´?øÄÉþ¼3"@*0aFÁÛ¿ÆǪ5¿à\¶úS¿á䠓ˆÞ`¿ß"ãÍy¿ß™Ì$0`ñ¿ç/Ç~fAGNrdg3FGL J1442.6+51563C 303?ïÄ:¦ˆÚ?'JÏmëY?Tž F±g.?YÆâ©`<¨?x»$½ÔSU?~ÈO²–Oî?/¿"Ý?"àYŒÑD?a)¹[Y®¤?a¹`ŸU,ò?‰ÇEÆ«?'ß`W–…a?ï"ó:'vÅ?s›`myè?`î³Gܵ¾?]–èƒôV?Š‡"ªZmE?póã1~*e?ï!_'"™X?té{—mŸâ?}¯Vr Y?_†7Ñ~^?"hGòDññ?tӛzô­±?ïŽ!‰ù¤­?'מ˜¢æ?d¡Ã¸gÂ1?_üS|:?‡O, ã^?€j¨qLA?î¿ç'õW?´þðxˆ?rk½K¿?tl½âÏ?¡´'o>Ÿ?œ†M¢|?ï.úÐ|?…ò~qÐ?iܪúÏà?bcX\'ô?™´DÄæs?ƒ\ÓNËÜä?í@Q±DþY?'ðšdù?"Ø•b:MR?}£3š?±M%`á?'aîMÃAGN4FGL J1443.1+4728¿Ãä8èî…H@N&ԀuÀ:k"Úí÷ÀÀ<¡´¯Ÿ•\@r*£Í@^ïCðÙ?¾a¥'°?ÈõæA½å@37º@Ó´Ï*8¿º^-ݳÏÑ¿å¦Ï!»¼"¿ç-O>+´º¿é©ŒUä8#¿ð?ïæþ!¯AGNnlsy1B3 1441+476?ï§2š˜-o?}v-Ø¥#?x=,OL?s¤×"›Žœ?t)†q«·Q?nL-"S´Ô?îwAÇdqÞ?¨	.cØÆ?"tO3úv? T¡xþG?£wÜÄ?—
Ð\‡?îö
X-=¦?dZ‡/ë?"‡[ñ ?'	ó
±"Q?–úÍL_»8?…á22Íʳ?ïfâËo]9?sâjzôp?‡ÞN?o¢É@?~rˆ'óþŽ?a˦Š*G?ï,»išoÐ?'}²É›ˆë?Œ»8CÌ;?†Cœ¦®ñ?ˆíKI3ã?†òžr»A1?ëǕ¡?ÀªüQŽÒ?¬˜[¤=!ú?·tÀ3pÍ?³w%#X¨@?®J*È4õq?íHVdªhc? £å¨øZ?œî֜`F²?'ñ20˜×?­.bÝӂ?™¢¢øU J?íÔ%ŸTw.?˜GtBN‹?¤ßμy#?'æ\‡Ã?›»®¡¦sì?"Ö)›CªAGN4FGL J1443.6+2515¿ëæK-GXQ@P4t>–=ÅÀ;-ZyɺÀ<4šöå¥@#

éw¨X?û½{Uá³å?Òð'ÿ¤:‡?­•9•T?ð'ß»¼Ú@­pՀ$©¿îÖëÔÏЍ¿ïþ(ßó>?ïû»'w"?Újµ ¶Cs¿Ö£D\¿àŽ¿`}™3AGNbllNVSS J144334+251559?ï}&?:?©ÿĎf…?KË«¿v?lpé_:ë?ƒI*~I?¨>ø¼$Ø?ï©CŒ-®? ihR¾'¡?Q:kðkÈÞ?a‰ x%ñ?ƒ‡Ï|0{i? -n%«?îÜÔ+ç?Ÿ;rk8'?V`¹)§ï?a©Ï塀?®LÌms¤Q?Ÿ2õêÔ?î;™€''@?"ó-•¬¨?LbŠÃ˜?C{¬³êþ?«ÔÝËúIE?"Ô¤,{¦B?ï3l¥+?
áÞÁfÉ?S"y ¦1c?P݌x¡äÛ?žaJԬÂ?œ{üíÕD»?ï´V´A¼?®±ùaÖ3Ô?_³)<ò?q"Œ¶èÐ?šÎD¤¨I?­}±Jÿ?ì()Ðð?©Šèê?e)*™`Ù?pàí£ƒß?¿EuÍY#?¨ÖÁ4–Ÿ9?êâŒï´?±‰(©ç?f#uàµÂ"?mÜÉÁíÝ?Äg÷'zf?±xg³­üAGN4FGL J1443.7-0954¿év¢žŽ@FlvJßøÀ:ÜdöúÀÀ<hô'
´@™Úk›…@\}ÿà?ÉzúÁ»!?p:ÙâãN>?¦¹ÉdãY?þÚÛô#`?¦É{ßto>¿éžÒ¾~Up¿â\~¸+¿àw@Ý?â¿Ö6h½ÕG¿ïúua«ì'AGNbcuPMN J1443-0953?ï9{⊵?'Žõ÷tˆ?X¬Vòt&?L
¾'/Š?—A‹Ä°?'¸ì¨7×?ïnÕ °å?†jϪîC?^ɃÇ>PD?`Ùºc™"•?ˆåZÄ?"Ñ¿¯m?ï9ýoVúä?Õ:yÿ?cš.$æ?Q[ˆÞ4x?–H%vuí?(¤½¥Ä¡?ï
µìq¾ð?s·
L§Y?dp¨X/?IêØpÚá ?›»-m?G?s#üWS¡Ü?î57~é·a?£õ ¢
»½?fãf}¹?X".ÿ|Œj?«KYÚ6λ?£«Q†h6?îíÆÉl^è?›&9b'Àc?jJÓSrÅz?sg½_h?žýÌnåQ?™j|™°J?î?>§¹¤?–¦æŽ]ß?q92ÓFK"?e–Çñˆ{_?©äï(MnK?•ÖœðÚÕ?í(ÄAš?''–æ—ìI?yBž­w?g"ýßÎ	?µ%µ›À«Ð?'"—éòö£AGN4FGL J1443.9-3908?Ýé30à@2µ÷øʁ™À7ë府mÀ;8˜Ä@\a¾¶ß?ûÃ/zA¾?œ¼åN"ø¨?¬ÇïBmÍ@ˆ®`Ðû0@ í6ϟæ?ïýÖ.u^¿¸ù§÷*ni¿Ûà«;'¿Õ'€áü}¿á8 m]Ñl¿ÓÜ.ÿò¾úAGNbll3FGL J1444.0-3907PKS 1440-389?ïÞ1k²Ö'?dô5±¼Ÿß?Krޒ!}ú?HàiòGÇ{?jñܼ?aŸìU9?ï,,è&«¢?œÓ¬€u2?aöÕ]ä½?^›·n%S?'Ég'‹]l?•Iø¥Ä?ïµMæN?"ºU™á?r–GÒÁ÷8?|Z°ú+#H?—ƒÄH®jm?'sÀ֚7?ìtÏäóùÑ?–¿X"ƒè?–[QöœóÏ?t+bçNUë?¶Â¬ZK?•çãYTø?ï¼zzxÓ?w¾¹Be-?Tyšß‹‰•?T$¸°°îg?|¤[ïàè)?uMdsZ]?î
eÓ)Ä[?®ãÌìÍá.?'• ;ža‹?œ`*ã™7?¦«I"?§©Þs•?îž|Šó—?›¥ÍO@¿j?xÛ舑÷Ë?'TâÙ÷&@?¢üº?`î?šAç>¾"?é©«h+Á?¨)©ÏYµ?£Œék•¯'?‹}Ü.&Ÿu?ÄvìdS?§úÊbăCAGN4FGL J1443.9+2501¿ïÿ¸~ÙqB@P,†hÍÀ7Ðe…•Ö–À;]ˆ{¯¤@ûV$#öª?ÿwÃ Ô ~?—	"ŸG¿˜?¹®œ`w	@!ìæŠ
5@ù$ƒmj¿½¼O?òøõ¿Øó¤·Yô¿ál¹–m•¿á¢9ìN¿æµ6]ŠÒ¿ç_û¹IbAGNfsrq3FGL J1443.9+2502PKS 1441+25?ï_ºJò $?°(\Ìý?uNΝnP?šFì5ŽPg?jaRaû?¥$ØG¬Ú?ï³®äb_?…ÀÇaÒ"º?^ºMÉK?zȞ€^Š?~z	B€?Uï2kÏ¿?îµê;.?šŠ˜é©#?´mö̧B?'Ï­Þ½=¢?˜©±&ĉ?"Þž)¢ðî?ïìaù!òø?RÜgØ×÷?5nA\î?+ðR9BÕ?`ýã¡ù°?P™L9?ïTÞ-"°?ª¿dޕ»Ø?rfý¹¡pV?'¡¼¿Ãà?ÊzÝÍÃE?¢÷"¥åZ?ïCÜ.P¡?˜י\ò?q€å´Íl?ƒ¿ø4xèR?"=Èhz?"snq(µw?îá0ç  ?˜³Úí´¿^?‡IHÚu"?Œ׿ËÛ¬?˜5>·\{?"42N—ú?ï͔´mä?o†—1s?FdxÃ:'??u¯eq3Ã?vi}šÿ?m°ñ™ô©ÿAGN4FGL J1445.0-0326¿ëßҋR®ù@Hw @|ÇÒÀ9‡9+
ËÀ;î¬yp@ å"aÎüþ?ù¶ï¶àë?·sJ$'YÚ?»¼LÞRD@Ôƾ•Òe@"N÷3þŠ?ÐÉ@üžý¿æÛ§r$¿ÐúAd¤Dm¿Ðí»Ú·5¿ÒK1­>½¿äv‡EÙþäAGNbll3FGL J1445.0-0328RBS 1424?ï`ØŒ'Á?¬îºïeå?`/Ëük–"?RªÞióÕ?'ßë}ù?¬ðøBtÙA?ïyU{Ú?ŽÇ1»
˜å?nmŽGÑ?}½0ÎÖ?ŠOR'Þú?ƒ[£›üLy?îvlåýu?"Û~VÍ55?Á§ÓÈC?€'‰ââý?¤¡
£³S?'±Úëää?ëV·.U?¿B! ?â	¼?nÀÍ ÂàÀ?À£'±c©Œ?þŸ2.?îQ
}…×?·"ºÍo*?|è̶9?Ž·|€šû?¢šò#cT?´
€ÈǗt?îi"Ô÷¤Î?£ð£æ={?ƒò=1ª@2?Œr	Ø|öy?¤k#f@ä'?ž×¼,%(Ø?íÌøtN?¡é£4\"ä?ŠöSü"ó?†#úá&-ä?³ÂÍ»V­? MꌮØ#?å¢u¢æÁ¸?§4"iÿK? vAóçÚ?‡tÅÁïã?Ò¬L{Ðþ,?§=¤G¿ÔŽAGN4FGL J1445.2-1954¿ïž½ÜU<.@A¾ýq?À;yåŸ+ªÀ<r`±¿Ÿ@öé·>E5@AƎÅ*A?Á&Ž_(Új¿¶û`‰ÆÕ?öRXâð$Á@Û³'ÎÒ?Ú'Ý¿ŽJÜ¿æCx$Õ¿µ7ýu×s¿ë)xŸN¿é*ƒ–øÕi?ÁóTöÒYÕAGNbcuNVSS J144511-195853?ï5úûª?±–úç× ?ƒº •+^Ê?°ÚôŸá?Žá 䘺?"ü X'P'?ïŽ.»÷‰Ü?‡²d­öã?dÁnEÂÕ?mžTÜ#?‡D
³ò'-?'lÑØVñ?ï»þô<R?µ<ªZ{?z¶-	^´§?óô÷Uè?˜šôæÛç~?ŒFšxy©Þ?ï&Uw´J(?xD§á›:?dÇCK[T"?QEŸìÎÛª?˜œhš·ëƒ?wáÃ)bx?î¤SÇRd|?¡o%åˆT?~ÖôËÈۜ?E0'dnÒ?¡ßäìÿU?ž÷rËv ô?îïBbÑ—?›j Å£[ç?pð
	LÇ?{—ŠÃalî?Û°aÔ}¾?—çP—Ù6N?íöZ>²9Æ?žžŒ'
Úð?"'‰O«&?…
$)Ì?«uù©QU?›û±°Ÿl-?ìØ©ˆqv?žŸé à8N?€^ŠÈCÕ?y‰äsk?·3¹[çîw?ó]½dˆAGN4FGL J1445.9-1626?ì#ÎÚKÄ@C(˜ëÀ9ìã.qÀ<õHG@°jœ€ÿš@•öâJ"?·`oA{P¿¡$`©ÛS?äg]Ж@Õ@–ÉÁ¿»ƒk.ø¿é–ãô5ǿ䟗_'œ}¿ä dŽõÑ©¿ì¨þoH?½¤òé.–AGNbll3FGL J1446.1-1628PKS B1443-162?ïè…ý‰È?^òÈJ¹7?M¢µ1çiÊ?EŸ4J½0n?`Là
È­?Y!âò^ÇÙ?ïÝ
‹Zw×?n6Ø"t¬?C¶pOÛ«?NՕÍՀ?nظ§Ÿ–?h"(WÝÇ?ïšÍ"ªÙ?ÒDࡗG?`¾É'rpm?e5;Ǒ"Ž?…«?}ªÏ8Å=ì?ïÙ¼fo˜?RcÈò埳?PˆžfáJ-?7‰ezÔ?mÿJÑ‡Ý?N´0gª·?ïÊ$P(ó?nǾ11Ýê?d4ø¼ Ž?^Tƒ&û?pÓu¸/Þ?gçÈ®‰…š?ï£FA5ˆ?ƒ ²HWSÄ?QÀƒ'äò?`'Ú\w»&?"ö_1,·ˆ?uŠ É?ï<¨Üúä°?‰ì®69ƒ?l…—ôpÝ:?q^øãEÿý?"Ú1`áqi?‡^c9j˜?ïŽÂ¼\ê?qat´?i¥T(‡?V?AwÜ<ý?…æ	ôEm»?l†´"•r6AGN4FGL J1446.0-3039¿íjå6َ…@:
§;BÌ-À:ó"PXÞÀ<nsGyB@õq´ùŠ@趽–Îä?ЯûIaô?Òcˆ»zêØ?ü|MÃØ1…@"Ì€KÀ¿ï‡Š¾4ƒ•?ï¼ë
)´.¿Ù©`J{¿èÕ@8Õ3¤¿ì%ƺd¿Ó/K²…ùªAGNbcuPMN J1445-3036?f¬?~úˆ+°¤?aÍ–•2?TÀ~nE±ÿ?ƒÞ¸Jr^©?{éT­'_æ?ïÔÀ:d¢?s1q•ƒ/V?K1ïõ8?W·ϛ¹¥?r•b	'Þ3?nod+k›1?î¿£9瓉?"DE·?ˆ	Ȁ·Ë^?…¢šÁX?œ´}Š?@?ŽS!%™¶ƒ?獵îŠÑo?aŸòLÛÊD?`ø"öÉD]?BT¹üïÚ-?'ã$hÇ??`FpC¶@u?ï84™c?ÉÇË
sÚ?sY¥›u?j¹]%ÂSÄ?"-#PEÈ?Š°°}b?ïyÙj"ôC?'.Ylž\ú?allJ(?oÄ1=$Ò?.ŠIH&?Ž!æ.ȕ[?îùzfÚ?›q ðê¨?'î´@Hve?Ž-CÁ1l?¦)6ç'7?"Óª=4?ï
'Œ.C'?€¨jAè,Ð?r1îãk«e?]D¬%ç?™Ã2¾Dþö?q¯y¥íAGN4FGL J1446.3+3111?×5Ç~"@P)ú—á2µÀ:¨ñ-Õ%aÀ<©Êbh@rÝ4y@Sw[0?À&ágc'?'ùXyœVÁ?ÑÞ¸ù6@û0ÍÓ2¿Ö¾ÔãÄ¿ßâ¼Bô/¿æ"º!N"G¿ì¦á€¸ø¿»ãÆÃö¡¿ïô½±¦×AGNbcuMG2 J144640+3110?ïúŒü?8ŵ7?"FÆ°w?'±øø?A8Ic·Õö?5.-€0?ïå¡ü$åN?k[7B¾>à?7Ë¡¨ØŽ?Dö¯%å†?glJ¦ÎR·?gÿz)×áÉ?ï£dt&v?w»–=twÈ?ZÌlÔæ^?aÞD›ß@?ƒÍUaE5?užøT˜9D?ïýsß±è?éÒ¯™'.?‹¡æMÊ>óä°u8*î?2ŽÌÉDÝ?êöœCµ?ïöS€ÕS?NÜy'‡1¨?-Ôé(¡òå?%:+ù–v?O>d*ç»É?L¥>û¢ø/?ï¯øöÝ~?"‹z¨ñ?G#]Áú?Uy
Äv?'ÈKì¼#+?'ñ²æÃØ*?ïV|øŠQ?"Ϻ;Ehy?j5îù™EÎ?r«ÕÔ°ãb?'ø²~£ç)?B&{IäY?ïøãÃÖ¦?=F³AF›Ý?2[kr½?A®9qx?Kú$‰ I|?;Εä´AGN4FGL J1446.7+1719?ïÖ'žs-@NÓ³áC|WÀ:²ìzçý«À<s›x¦@Lȯ0ړ@äÖä}Ãz?Ä#-¡?¹zþuÍs?ðítw¡!M@–më?ïá\Üyèú¿àH8³¥´Z¿ì4á=òÿ¼¿×—ÿ»Œ‰¿ë{Háa«¿ðAGNfsrqS3 1444+17?ïí^	Bq?U´nØâò	?Ck'­La?8¹o÷h>?[{¸)öø0?R
ojù?ïށHÑe?mó
𽠖?A-÷µ²Âž?Jµa"¤Æ?m39o®‹?ir҂?ïmîÌb)ý?‡T'®©?r+­í~?}²Ž…°ØÌ?‹<7—ã"?'ðصÛ9?ïÝo¼üJ>?Pr&/};?X"7Û:°?@l&X×?fF'ª?IÄ£Uññ²?ïã±mé?a­I«@õ6?Qÿ'Æ»kŸ?LzÓ>yÛ*?cê…##ÉC?ZñMøM‰?ïÇ­—í?‡öq!ZŒ¡?VÏSÍKª?aI£!©¿?‰´*+²^?…Ö›
e'4?ï@Vv,?>'JœU?y½5nQb?}C'\¼IÂ?—ȯ]…!?‹uáµer¹?ï'CÉzÕ+?pxþÛ)?uQnê?d–¬?€®‡‹#Ýô?gCÕè3kvAGN4FGL J1446.8-1830¿¸"™Oäµ@B;½‹ç)À;·ª%ÙÀ<†šÜ¸o@ N'?ØÞ?þsŠ ÒH?Óû–
óފ?°-ÜP§?Üٗ ¢‰@—ñ¥]¿è=.ߑu‰¿å©ÊiE=ø¿é¨@[9âz¿¹B	岿ҤvÂT"í¿ïú Ë®AGNbcu3FGL J1446.8-1831NVSS J144644-182922?器ZúÍf?…cל²ÉY?AÀsKÛi?;fINí=?"Á-B"‹N?"Û`Õ¥2?ïÑÊ}g3ì?qÜ­8´‡?B]!œøÊ?I
[çõãr?tÏ3Àju?nMñ™m¡Z?ï\ïüõ?~ -Í׆?`Р½_|~?T÷Œh¬…e?'GìM§šè?|õµ	EÓ¼?øc9Ç?j#üh)·Å?E˛'IƁ?0úiэé¶?ŠÈ>3ª?i×qè6÷ï?ïc¿úε'?‹O&'£?JŸKN ä?Až¼ó]?'³N¹ü…?ŠÜRIû€ý?ï'IÍÃ0±?ˆ}?Ÿ?Q°҆çè?Y˜è)FŽ?7‹ÁñzÍ?‡PV)_þ?î°¹kq<?'UFøDÇF?l$P5g–?fÅP€Ìõ?£2$KB?suK9Aô?ÕF™?†GFÕ@Rš?W¡°M"û&?O‹zJà€3?£â¸¦¨•?†
GžÓ~èAGN4FGL J1447.0-2657?ëûÉýQ@=09-Œ*À;‹;26À<—)2ÿ0Í@ °›yB·
?þ³&Ó©_à?Ç£ue‡Ä/?ªugáÏ×?âNæíàBË?þ³a'È?è%¼£n/¿ïÿÿ)@k*?ïÿøsCÄ{¿è©ý·{W¿Ù,ëñUB¿±Ó	&ð.ÒAGNbcuNVSS J144657-265713?ìÒí¸ª«æ?óS^Ì¿?G‹ÿÿ9Cf?B,î
‰ný?¹9z;ñ¢ä?ðÒruŠ¾?-ú?‹"'žœ›~?eŠ¢à/;?lûMÄ|â?ˆZk—Žã™?‡g¸í[?ì^‡9Ş…?¯õ1ltøn?^‡íº,I?_
 BÓSÂ?¼'¦}z ¥?¯÷~5¢ë?îÈÜhSÙú?"ömv!±?jBñ·}Þ:?`s—V:J²?¡Î
bÐñ?"\ۄš_?í?»	‰?»gö‰^¸ó?T,ê
tžö?Xk7O…Jî?¶þš[Rºw?»[*Þzõ?îÞEû.Vw? •õŽü¡k?rÖØa>(?'^j´ÒQ?Ÿ¹Ü½¡?œTˆy}óµ?ëºãï[ˋ?±]=Uê?f2WRS?g˜'þê$?À¼Wz¡m	?±bž~fÕ?ì¼S9Û:p?£)s¥jèi?zî•]"E?{vqÒ"r¬?¸n|Ùq*M?¢˜Úa£'AGN4FGL J1448.0+3608¿ë5,`õÒï@OÛKƧïžÀ8é™ÛøóÀ;¸˜SH|q@g.†?ù˜Â¤TÞ?ªF-ƒ=Y?¼üë"£C@¸á]}Š@	¸¯&Ëî¿ïb²|¿n??ïþk«IÅF¿Ñ)õœÏ®ÿ¿ÚGž¿Üí:*ž9<¿à®!`¢ØAGNbll3FGL J1448.0+3608RBS 1432?ïævÝø;?bž™8@ÓK?V–SlÐ??WãDW¥²Ç?\}¦qŠÜ
?SŸùb?ï)î2o‹K?ÎKU}…É?'|wØ#L?"æõ@5L?'ƒýÈdªœ?rö-Ži?/^½? Õ˜Mi?_?›4(j#;?˜¯¶ê¸? Ê#|ÁM'?–üÊüöí?ìÛ­}|,¡?–QqÈÖYO?˜€¯ÎöXó?}=*8Pê?³h"Ò¶?"Ѭ=\Ã?ï¿¿—w3?rä}âf¹‰?f蔵Îha?byÎö=F?t¬2æk¶0?kiÒ'9à¸?íñÇ꩛^?¯99§:?'"×¼(µ?¡¦7®4^Á?§™•sâS[?§i=|D?íÕKøb8?¢¦PƝÜë?ž»µñŒê?™Mb©?£Meì†>?›Õ/qݒî?êFƑ'è?©ÓOóQT?¢~:Z©J»?ŽýΤ½A?ÂEW&qG°?©'?ϗ»AGN4FGL J1449.5+2746¿íŸTª.ð·@OìÏÃøÀ;ÐÄv¼õ¿À<øV6mzW@"ox.åƙ?ô•|3WEa?Ø\Kz§»ñ?Ù]لÁg@¶ÄŸä@µréµ?¾¤çÀîó¿ÝI¼ÈÊ?ïýÐÈÚп¥´£5NÁY¿ÒT9]nÆ¿ÛîH}GS|AGNrdgB2 1447+27?ïhªðÑ&?Žúǖ]ù%?bæ9È]-V?[KXµÐQ?Ú¯Ê™¨?Œu:GW5$?ïw_ÏbB.?AY#£Ae?hká[ïNá?poÄË®å?Œ
ز°­?‹b‹Ïý9ï?î.å{ob?žb·™Ú"&?u=v;DF?xy8‡Ò8?ªp œª0›?WõÓ	?íÿçÑé?Ž3*֖›?n6$4SÎ?_ĈW•?® Üå­³?¶X•c4?ï,æô§m~?•‡Bìô‡?næßâšÃ?fÈÛËø!s?–†Ef×ôu?"(ißhY?
`?¨Å`³#Ln?zE#–J>D?…ÜÄ'î?¤
:³×ž½?¥J<ãŸÈ?ìÝùË2˜Ú?§ì+Î8•?v"Jpeê?xµ@ þé…?·§''•?§¯tiŒË?êÔ¿^iÂ?¨õíæ™?uÌ#ÃÍIr?tí7¿$?Ãþ¡hƒ­?§ÕÒfâ¸AGN4FGL J1449.6-2137¿ï²H#±@@¼Èÿ¸²dÀ:»I»4ôÔÀ<Kžã…uö@çk´"@eäEVJ?Â-`‹[¿«9s'óS¹?ê†nCªz@Òùæ‹dο×ÈçDÈ1¿âìÊ-¶°¿ìÉv7]d?±å/D;CM¿çRw@Ý@¿ïÿ‰XAGNfsrqPKS B1446-214?ïîÇ\å"?UìÖy<5Ÿ??x´3Þ/Ê?4¡
ÔçTr?Z"£sbÒ?S?‰Å˂ž?ïæ«Ñ]2ê?iw¨øñ¿?8XŒ€K
?CÀêÿ´?fIéê?fV*" 7ï?ïb²"C"u?xdïØ?Y}éÁKx?]4 y:\%?'ÐÕ'Þ?5Úø÷‡'?ïß|úsña?R>ÅoVÁ*?:]£¼õÍ?%Õå)íxF?m7eèT‰?QZ•-<cß?ïçó2"x6?b¯\k?Lq[|g?I-:‹[Ÿœ?`ð‡EeÜ?]í[wœÝ?ï³[*6ú?€‹´gôۈ?KõOÇA^K?Vâ¤zË.±?zÔ-#"«?}û¹JÎØ?ïi?'?EÉî?fÅ3ä#¤¢?oɈ'Àt?šº6¿|#´?zBÖDm?ï"Lá//n?tb·áRrÃ?\5'Ñ1?SáÚŠÛ?‡ª€÷«*?smôKØÛAGN4FGL J1449.7-0910?ï+RßJþ¬@EÞB||RaÀ;)!°:À<‡àmòL@ >1´Øå4?þ‡S–€	¦?֝ţ7Ó?»Ž-TÌàï?êð äÑü?ìæ¹ÏçV¿ì§'Z¸³:?ïþ¡€Ã´Ë¿êéˆÅ5ÿ–?³=ïϱ-µ¿ÝÐ$p!Ñ¿ïÿÏ=ÀTïAGNagn1RXS J144942.2-091018?ï•)qWJ?N'¶àÍ?VEå%×Ւ?^Š'?`"?‡ìç	ê ?Ž÷Sj'"ƒ?ïýbäC?‰˜p=j'?k½Ÿv??w'j>Ï×?"Ñ?vƒ,)?€S°â²-?îÉjêÚ~ç?"Óé}…Ýg?äè-˜˜?"«D•Dñ?žC°6œ§Ê?Â¿8?íínøû]?°·ø'=ÿ?'­—ŇrË?{0gç€?¨RS @EÎ?‰-‰¬åÇ]?ï†zé*Q?ö#ËE¿ü?` ïk·ç?iA6‰Zƒn?Švev¢)Ó?Œƒ5[P?NÚـ?¤plÌ}Ù?"¯éÔ"ä?" òw'ø«? ÿ?±Í?œvÒGʔÅ?în:×S?œÒ%oOl?T*Ÿqçý?eUù‡?¦²Þtv×?–B9ÅÐW'?듓êœÛ1?¥)e9v¶n?œ¶OÇcbm?"zmî뼙?¼5Ì·ös\?¢ÿÁí6AGN4FGL J1450.4+0910?îçÚºv3
@LT°ò{²ÿÀ:7s	â×ÑÀ<e …F%~@´—Â;ú@æ3
9?Ã
'åÍúŸ?ÅëX¦4]@&¤û¨'@SF¶È©}?ì!åbÅÇö¿Ù8¸ãá¼H¿åÍà¿åq•n'¿é{NP¿ïìŽ:AGNfsrq3FGL J1450.4+0911TXS 1448+093?ïßyúº=K?_t1Ü­~?Q•ëŽW"?Eå›%öþ?g»}òW¡?XÕ–#f6?ïØX74Û»?pÁÒݯák?EÚ§OP€?P–èøôÂ?q‰Æuï?k¡Íi…¢½?ƒŒ"?sHróF?f\¬›'f?hÞ<Ö³ø?z³þ´KX?lõcƒ"?ïÜWJÙ[ë?Náoj|˜…?X'Òœ™Ð?<´HÕºAš?g_Lœ…?G²9ð/7?ïÃ	¥£Æ¢?nùõQ¶¹?`—¯½%š?WH2EbåÇ?v/UnvŸ&?h•Œ}–u?ï'	ӛü~?†FïÃ?Y@™¾N¥?f#Ýðؐ?ˆ•wîEÏ?ƒ8êû‰•??ïE·‹-Va?†Œ>¦Ô¡ ?u´üãÌ0Û?u°µÆz?'ÛÏf]–¯?'"üà/'þ?«K?kti–jÖ?n!ƒ½ú?Vu†¨Çì?™èr'h&?fIBþªAGN4FGL J1450.8+5201?Öùd•<#@LEåóöÀ9¯UªLoÀ<P)µ/ë@7Ž`U€:@ ÷üü??¶2¬`×ÂZ?¼ŒÛ›Ï¿@5 üÏÊ@£þ·Öp?í/B]r¡Þ?ÖؽÜD"¿ã&??#€¿á*™Á²'d¿áÚŸ‹Ëü¿ïÿú÷''ýAGNbll3FGL J1450.9+5200SDSS J145059.99+520111.7?ïÅóÝ»e$?f¤·Ì^ä¤?\(ÙêùÒÏ?Ps"ñ'´:?uûÚ¯E?b߄}U4?ïØ´LÇ?—j¸Ž/?ƒŒÇH³]õ?‰*/S3?'ž…Þô'?Š>j©),?ïFú¸˜bb?†±›Ý°c¤?xƒŽÂ´pº?|ãYoG·€?ÿÅ@¾?¢´ÜÔIs?íP®n<ô?Ž´Ènû'­?®E#«ÃÍ&?Š€™hRl? ÑmXc'?|ŠMÅ´k^?ï†qúvÜ´?{UÄqxW?q¡åe›ur?f(‡âí?…'Ž£Ìlb?u8œ L?팢5'2?°ŸËü‡t?™r$Ëìq?¡ß¸üz(T?ª…yK	X?£ÿ]"kîw?îhá=G3E?–zœCçH?‹	.–°?‡¼ê@JÿË?¢¯ …Üë?Åi+<Ĭ?éJvOµ?¤¹ÿw'Sq?ÁƒÔ3QÕ?¢ÒVxb`?²¨µ«P¯?"‰¬Œq…AGN4FGL J1451.4+6355¿ïÚÄ'.:@H:A€ÓÏöÀ:ƒŠc›±À<¦p‰Õ×8@ "6}•'?ýNQÒÓw?µxõµ#bÜ¿€ÂZï
®?Ì©3€
&u@à±F?ækҁA³ÿ¿áŒ&ÿÉ#u¿ß S<h5¿âˆéH-–;¿Å€¢è!çܿʹÁáAGNbll3FGL J1451.2+6355RX J1451.4+6354?ïõõ¹Ò?EËFPnÀ?-Nò{5ö? Ig±µl?R,6Ÿd?C`»ڐ?ïã¬Âì#T?i"iK5Û?8j¡_?DPØDn?iEûFÄÜ?eë
õÜK?ï_-"iÿ?€qrB™?S(M"g ?`Ô%¾KñÃ?‰Ã*ñ÷ýÉ?Gò-쎿?ïÙÍ#LÙ?SÅv-bž?:zV#}.n?"n‡YôB…?qq×ñቾ?Sl qŒû ?ïæïT•?gZÙ­ÂXÈ?B=i£¢Óõ?B7^&Ù?d‹*us?d-üå³Ák?ïŽúî&?Î^Éï4Ç?JÊԒÒt¾?Vî \Qr?ŠÎÓ÷´8?ŽøˆqÙ*?ï+ÿ/J›Z?‹@É褖8?XÖ~Ýñ¯P?X`Êÿmâõ?˜ò²%çÙ?‹'•üþ"?ï~7Éx?v¤OjŒi?T>¢ÓV55?EªšŒ?Ô]°wf?và.ö¯íAGN4FGL J1451.5+1415¿ÆÄÀ†9âÇ@M›ÑþdõMÀ:ˆÒÿì´ÊÀ<wí4Ka'@'{yž@ݖÁxô?Å{>û…i?Ò¾ä!'B@²• Ž@ë¾(DAοî‰þñã?·Ð³Œ4c¿åGªfpw¿èOø ºÎ¿àLèyÑ¿ïÿçvœ>AGNbcuNVSS J145126+141626?!?~BL~ÿR?gå&‰ÑUk?`ïûaۉ?ƒ…"[Ø@?xå碌PA?ï¼BôÏÓÆ?y+è×ëqý?VˆtÔÐU?]0([Ò°Z?|<hdc?t™kG?îíìxÑo?'D©‰C?ˆ(ûiàQ?‰'HíYµ(?–.ã7™á?Š³œ{Öx?ï]ñïfC?mûzEԓ?~üú³×?aØ!g?ˆÄ+r‡w?eny=Ú/O?ïѨºÚî?•‹q݉?{('0›ñ?w®¥t52?—›¦Fø£E?'ò¤IaM?ï­³ya?—vSz3c?scõÒñ?xPxbB8?˜Q"'{'<?"Û îr?îA»EÞ(?™Š\6xS?§:{'Ö?‰á×*[¹³?¤z}"û­?•<Àê©G?îá^,(?ŽÒ(ztD³?™#Jëˆ:&?ƒ¨5ð#'p?£0Hµ5r?……\"¹1¦AGN4FGL J1451.8-3851?ì;—±É!ƒ@2FìÔªÀ;qߐô¯jÀ<‡ªhô¶ @ þGG<Tš@gã'ñ·?Ì+ýß¿BÌ?{E"ï¥1?³\&á/?@Ùt·b}¿¦<!•.®?ï[›fù3]¿éÌewS¿Êz:ßO¿ïÿüÚ±'Þ?ïÿíÁ9ÔAGNbcuPKS 1448-386?ïT"|bëÌ?"_ã"ã?rr{p‹?ˆßÐ]ñß?Ñ
™íï‹?‹ãKv+?ïzfÇùî?Žaã3']þ?h',ôê?p´+h&§?‹B	µ—nJ?ˆg/:Ê?îBàÒé?˜é}ÔäjÆ?Œ-|Pb·é?‹:X®|[™?¤Æ"¿éN3?"!<É["€?ïO{Aã?€b1I¸S™?x•À°ËÄ?dÊHèÃúž?–PÉ«Œ­?|^ÏNøWµ?ï%/ÄS?–Ò1^Én[?zêäP'À?'1PG|©'?"Ÿ—T.ò?"ãç5"í?î¶>AÜ?¢Ãi§×?w¶K'òÓ?…Ö‡ªíí?¡¥JcÏ'? öBé"êÊ?í=3l"üø?¢N,Ÿûpj?‰Àëd‰ä½?‡ªIÍÐï ?²ÞG-….? þÂãöÒ2?í)¾dæE?œÍëEò?'$Êî?ˆ_Ó{òҋ?²3pÛ¢b?˜â*4ºzmAGN4FGL J1453.0-1318¿ì¨¾ôƒ0]@CøŽ£œQÛÀ:Ó Z8[À<Zê'-@Ô®¯Um›@^pc?jy?Ä:šE;¿ŠðÉZ7À?ÅçúîHH@ñp;Ò>&¿îPáϓPª?ڂRÀ—4e¿ìJ[¾l·¹¿Î0CÐí¿å/5B,P¿ÌT—œiW²AGNbcuTXS 1450-131?ïeÎÔ	®?ˆÕêDçA–?[_'8Ù?P¹£Çê=¸?'4.õz°?‡÷Ÿä¡u?ïÚ7Wâ?n;Ý»?C…<«k¶?KÇ~ƒE?p™SËq"€?iGè
#`Ï?ï$ :nL?Œ‡Ý­J?o'󪫓ƒ?q4+dŠ~¬?—‹ý~åF?‰š*"ýHX?ï§Ä,ó±œ?b
9ìÂ)ë?ZÑLMI?@G}.­t?'˺©`ÃY?`'½xA=a?îÛ×¼È{?­vIœüÜ|?sÅï™Cž?ˆ"¬~vô?Ÿ¬©zr?§Î'9†Þ?ïŠÕ²M?‰®ÅÜ'?S
­Í=?_´ÏÕë¯f?Šê23:e?‡ýØòÕ2?îqõ%-â?"Ó¿¼5S^?yžÈÿ?w®Áó¡?¥¬ìÕs#?"·	8D?îöÇ91q_?¢:G¥ž?t¸¶n?a_³€]Ðñ?›ùèq?€Yœ`>ËAGN4FGL J1453.5+3505?âÓ£ç·@Oeì,äd™À:¸ŽS™ÛÀ<µ™ÙZyÉ@#>Wÿpc@X*™0¾?ÄeqH턨?²´rˆ2¿?꿹SsD›@Z(*¨3?ã¥L?ə'¿æ]4Ä,ë¿ä½Ø"kdÓ¿á»2Ál"¿ïæõ½†Þ¬?ëñø¶Ô"AGNfsrqMG2 J145315+3506?ïçÙù¹y?€EžÏ©@?=wùí­?O}Yb¥?dwؾ?|Ѕê<U»?ïß©˜Gè?q{'ϸ÷??E¡Nî?K5{Dû?m´ [?må°1ÚBT?ïŸ8³‹ïH?Lôr~²Ã?c'"7á?gúÍ
Ö׏?ƒq.½úö?{wP‰ÿI?ïò"µ·ºõ?<º6–
!??ó÷Uÿ¢?&Ɔ6˜#Ê?Rٖ¡z9?7szTïø?ïÕp˜ÕŠ?pyïwÍ'?HŸH˜y]r?B¼H…m<³?r3ʞÓw?nIY¥ä±À?ï›7Ê­Éã?†\te§?Qkö…ÇA?_W¿¦ëß?†ÿÿʾJ?ƒîí¤Ù̹?ïC?  i?‡Å¦CÊOÝ?kIöz7'?h)—«fKh?"$¹4ùã°?†Ðö[?ïÔOáG`Å?a¸jü3?XîødL?H±¥£%Ž?o¦'s˜ÈH?\2Ä+?TAGN4FGL J1454.0+4927¿ïãݘ›Ê@LÉÛ"Ðå`À;Lë8ȞjÀ<ª"Y–tK@"…|V'@¶LãÞa?Ó­Cðo¿?Ñ#l`üD4?ùìúÕÔ&@GÍ`Æi?ïõðaýK¿æÒ¬X4õ¿êÕï ·E&¿ÜjÃQ#¿ïñ'L ¿ãÈÏFúTAGNbcu87GB 145232.0+493854?ïÜV̯4z?eÑ:14™z?`~ÿºì¿?Zw[¿aò?c*3pGù,?XÖ¼ï™Á?ïl¸ø&T?ŽOÖGt?pôØ?€Î9?u_zßþ+Œ?ŒWUÍó?†vѲS"•?ïAØՙ¥?‰²-EOÃÌ?{go<DÅ?€'Ê|
ã0?ë	®×†?ƒ®ò2kCç?ïb6ê³ù¨?p2gHËD?{³¦TÏÐa?_öP]tR?‰˜r6°¤?j¤û	9§N?ï¬84FP?xz¨Èúšç?s‰3`µÂ?k;#PH4?vZ²ªiüð?p,upº?e¯(Ä?¢§Ý¹Šùä?€}Êëýé?Š

H]ª?¢gBõÂ;?|÷È+±?î¶]Š¨B²?"½bg!?ƒÚ?õa+?ƒÁœ
+}'?ŸG.¯ï0?)+–ˆwp?í˞k‡ÚÍ?'ßÿŽÓÞ]?–Ò5­¼`?ƒ(þ798l?§Üþq€8?Ž±Ž'å".AGN4FGL J1454.1+1622?îÊb		"ý@MÒ*¡"9ÞÀ9ÞúŒ"¹À<Zjۖ"@OÞÉ# @T[òoÅ?»Ð 쉬?Å`€Þ·°Ü@žÒ¾~Up@©§°Å?í>aå£2¿â¶œLÒA¿ål(—9¿æ:m"gÙ-¿ëæíª'æ!¿ïýÝÑ×ÏAGNfsrq3FGL J1454.0+1622CLASS J1454+1623?ï¿õÛ±8"?pÝ·ç#A?g´"Ìh‹?_j#y·Ö?t+0º±?gªáºj?´ÎÜÐ?'.M¬Äa?h
B&Ü?pî:َ\ë?'ŸOqppW?xZk÷?ï—w"ß?€úUsŸ?jеq´ËÁ?pk«
Œv?ƒn
/ۓN?z7`€Ô"Ø?ïN©åÛÖD?p»6LJ?ŠQUÅ?i´Ô‹òŒÜ?'m)¦zÿ?`'Ö­'c?ïh#†Ü—_?'"ϯ‰8?å^zôçÃ?uj<•Ï¸ú?"¿Ê®†?wxkнd?îìÏ*cð"?œŒÔ&lØ?|™ˆ»œ—?ˆJúoàG/?›?¸|³¯Å?•yvç҇ƒ?ï/[?õA?œe/t?€¦zz/÷?€C%¦þ"?"ÁYèXã?‰SºxJ?îô0Ûâ?Œj™'¾?¡ø‹
©Š?‡yÂh䨳?˜±@cÏ0 ?|#¶(YAGN4FGL J1454.1+2647¿¬4à³8Åý@O[2ßP]À;,7–oCÀ<°ÛE5"7@ØâÇàÔÂ@çÔÅ¿'R?ÆÛ Ña?¤Æa½y?Ù.$Àÿ?óT³.@?ïÉ,.\4¿º–ØÊü¿ãp,¸Å¯¿ãd¤úö«Ã¿ã îA灿Ö÷u'c/AGNbcuB2 1451+26?ïu¼\^?ˆZ©!Š,?]ÁÙ( °?TÇPS
m?ŽØ­Ó"×d?‡dN'8$Ë?îßD"غl?dGŸž7Û?ƒÃ;}&jÒ?Ž)¬¬µ?š5Ï̄É?"ºµÿóï?ï.䇲 ?‡$'•û:°?{;ÞÂ1'?}P|-hS?"Tw^Wåt?€è[¨Û"?í¦«ÔdÆ?‡²A7+0?E¶Ø³Ù?~DŽDdÖ?¦ògT秳?Â ¡6€?ïpÅK4m?''F'øâ?k¹‹0.Û?cmg–Ïã?šúµöîõœ?'¿ÆÀHxø?íxU§&u?µ‹SÖwä?—žE5½? ­dq"?±µUч‹i?®ï7Zà g?îw}š,?"&_WÛ³?ˆ=$Otð2?…\oáré?¢€Fqµl6?ÞÞd}B?éÃ@ܗ¤? '~V9»?±

os8.?—A۞uE?ÀmøÌ/?œe×Æ&cAGN4FGL J1454.4-3744?§—Eb|û=@3ÄüóÀ9µm¿öûuÀ;Üz¤áÌ8@ Ç†>@Ñ÷" ³Õ?ÀVË~C&ñ?É«ÿbKN³@ؖdZól@cô?ïê<´¼4Ï¿år†?tµ	¿æƒþý¡€ï¿çñLÝÙ¿ï÷Œ^G³ô?ïeÞ×sAGNfsrq3FGL J1454.2-3751PKS 1451-375?ï×'ú‹C?ss…õ¬ Ñ?d€r((úˆ?b€i{%?dkû˜"'u?ië_ŽÎ?ï‡ÿ|ï·?Žwc;%¿?qW‰ôFú?'ƒ[›?…qÔI<
Ò?<B¯\¹f?îç'F?"Wz¡mÓ?'W{ãu?JØ ¨r?'ÈãŸ|P–?'ˆÌQX¶p?ïTš3ûã™?s¯ULG?sÁ9Õ"Ú?Xá"[Ìlp?|ko3Ø?p\ÝG¹"?ȨÊ?|©üqôC?|¼–'¶Íó?uT1ÏÀ¦?r÷÷"!i?jÆ¥R¡ÃÎ?î²Ç´›9?¥©á*éb?ƒÅ–ÛJÕA?'"F£X÷?ŸÛ¢¦f9? !‹[Œo?탉e! l?¡é_ºÀ?¥M[YkKë?œý×í++?¢zWbL?"(HÆË>?í…Â{~ë?–lº…¥Ûl?'¼‰B:`o?~—i¿êlÂ?®Q_8â¯?'¿[÷¬Ý4AGN4FGL J1454.4+5124?îš1i•¬@L9Âã>ÿÀ8«]|OÀ;pêWøš@"3¬?ÿ~"Ô]ºÆ?—Ù~¥¼+"?¬f¸#{ï@¹¢ž%•@ô½:ˆ'
¿Î4
H®D¡¿Úp.›ô½­¿áßÀà/€ ¿ÝâÉc`Íu¿â‹ÑŸÅW¸¿ãë[-M@AGNbll3FGL J1454.5+5124TXS 1452+516?ïó)4y%Ó?EVv½è™ý?>ëÛûÏ?1Æqyep-?QüÏÓ@ú?A¾VÈ܁?ïÃp-B6?vlŸ"žÒ?NÒD€ç¬ÿ?Ui"×_»8?zm Ä¿Î?t|ÍPkUv?ï·j˃/?§lûàf?bÎn'û´Þ?rmMUF?zãbäôZ^?z'"dBó?ïÝs{LÒl?S> «š?H®vF÷G?1%%<ÚËS?l‡Y2›½œ?QT·s¾x?ïïkç?SŽ( ÐÆ?9ô¬4ÄÇ?21Ä5OÁ?\eØB¿÷¶?QôkÈ^&Ê?ïS5èLã'?'a	¼3¥Þ?cêBwøuÏ?nŸ,š&*?"úŸ}e/?'¯›çç*R?ï¸IRâه?¯ªd¼À?`^ž't×s?p¬ýþãÀB?{¬Tçô«?|ÂE$§s?ï±[>	º?oxn—0Š?[X«@_?J ܁1y[?€>Lþ€?lf{;·õ{AGN4FGL J1454.7+5237?ÀqÚ¡)c"@KÜýŸÓo~À;=*³1ñÀ<Ö»ÉoJ;@
—Éà´5?üË;¸<òÐ?Ô¤Kc֔!?ÝuX<8@•0¸/@9Æ7‡UÊ?ïÚ6ýÃÞ¿ín_E°¿ÈÒ<ã¶^¿äÍ _Š¿æó|†¿ïÿû˜'2AGNbll87GB 145311.3+524904?ïK'ì-:K?•:§uï(>?j{o,³ƒ?\évZ¶'?"K"–	3?"Ç}¶Ûl?îBÒl7Ðk?¥—C;ߗ9?"€$`Y?—õ²ãÜL¶?¡'ÇVk?šÃSzœ"?î_Ë$´à?•/ôX#z?†h.ˆ)ô?ƒÑä¢û?¤iB7'̇?")ó´²?ì}0 íÜù?'Ž½ÿq¾?¤œ Tá¾'?"½õ½ˆ–z?±È*ÍDR&?Ž¤3þ#?îIPÝN`q?¥¨†m(2µ?'UBSkõ¸?züŽSA%?¦Õ¡"«F?¤­""É‹?ë<'kä¼?ºsã–V²Ù?«¤°LY7
?°`(æê_y?¸IgP%š?°79c_1$?ìÍþµ§?¤°~Mù
?"'ýÁyl?‹ïÓùAþ?´¯JéáA?¢n_q9/?秂&®Ã?©Ìú²?±[xe†0u?œªl+ ?È´;4Î,¸?¨¢$ñœ`AGN4FGL J1455.0+0247?èÊôŠMm¾@IÜ¡ô±îÀ;¢oþDÀ<ϓ¤£@ ïþ¾âSr?óDƒ½B(?äF
<ã?ïýfÞ"N@dä]ã
&?ô†²+‹Éø¿ïÿ¾ýq??ïÿò~#¿?9Ár%·I®?ÖúÿšÕXâ¿á*Ä>³Äé¿ïþÔãÄAGNbll87GB 145233.9+030210?í†:òø¹?·ãsϧêã?Þ'ŠÃµ?™…*ªV2ð?¯-ÈfÚ¬?·r6Ñ%áŒ?íë-œ+«?¹IA÷Ο?¥¢Ì®zïc?³èÞÓÄê?¢>€xž<æ?Ÿž¼ 4%?ëLô²ÄãÊ?«}w¢ip?¢
4ç\Rä?™?³=<s?¼"?ø¾m9?¨Ç°òwM?èþ½e¯9ò?ª\¨({êÊ?³¶LSé׸?¤¹v›)?Â)ä=_d?§–ra‹$?í©ÁÕwì ?³ ¸ÿˆ?òáž?¤ë'3eKù?¦àé4Bš?®ä¤î'U?è¬	]CIx?Ê´»çß?Áj
Üc)?ÆáÙjP<?·ËŸ\±n¾?±ìRÍM?ꍠ
jæm?®™Óp¢? ˜
t?–®ˆR`?Á¥™Èú–p?¬nƵ›'Å?å#.A˖0?ºÆÖíÑÃñ?´œv'd"?µÌ&²úa?В£^rÜ?º|·5¶ÆAGN4FGL J1455.4-3654¿àúA-á~y@3£åÙä"À:K°¡šÀ<Ž`€s@±®MÛ«@ç]<9A?ÁPrß­?™Ôco. ?ÙG…5@èe{.õa¿ê6Ù{0øÆ¿ã'^aŠ3 ¿é©?^º z¿àþ壞U¿ÝhÚÆ_ ¿ëš	`ÑÑïAGNbcuPKS 1452-367?ïx`ñ Wþ?‰í¦!5r?a±Gd³Rç?U¹"ù7º†?{qës¹³?ˆ×(&øR?ï¹®Îá¿?ww|‡Ðq?SÃæ¨ÏÅ5?Wûˆ×<'á?~7÷j;§[?t#wB¬Ø?ï	ŸÄ‰?Œa_ˆªÄ?tláÞärÍ?s§uË??˜#"½"N?‡lž½.™ý?ï*§½ƒ{?r14x~&,?byóïúñó?EqÓÙ8Çn?˜[ÉÊüÍw?q|ñ'`É?îÎ}$!"?šUZXÎa?yÐêÃÌ«¼?p¦"Àì?Ÿ¼ ¹%S‹?˜œeÂJ¿v?ïEóGñíT?'é…ëŒ?c¶fô ºA?kÛî¸åÑ4?"ÊÊ"ªM<?'½øœÔú}?í€ÆùM?¡ˆùvÆR?Û:®·!?‡\';×:?°>gїÚ?ÔRëï?íl›%æ?'Å°~H?~g(º}¤¤?h;5g'Ç?²´°õˆÃ?ó'÷¸*KAGN4FGL J1455.8-7601¿é5îñ(»zÀ-ñk¹Œ~(À:ÞUNæíàÀ<ß®PàÃ@ ¤£e BÖ?ýóžÈ­ƒ[?ÆÛC]!ï?¿–ºÂM¬?óËg†ø­?ýÞU·¿ãLÀmBùz¿èYõ_45¿ÍáS¨c¿á¤Ó‰p#¿Óz­%²Z¿ê>¨çë6DAGNbcuSUMSS J145543-760054?îÒåõµÌ?¹Áøàü?TÓ&ûcÛi?o§¤f'¯x?¢+nøõä?¹	›p?ï|Í"üm?•ý«™?b±rq?hÇ A	Ô?ŒEµ{S[½?"ÖêÅÌ¡†?ï`ò×Y?6E´Ü•?_U°®Wš‡?X'źd?'ìaòÌ+`?~Aõð?î*¢<DB¿?"­|—®œ†?o¦Ž@hY"?Wpœ&:?«[s[Påt?"›D°f½?î¨e†¹åa?µ?´-Á?dƒæ)Ä7f?{²¼þhJ?¤1i/s©ÿ?³"Œó0ß?î¼¾Ü-"?¦ò11¡Û?oQÆÛÁé6?x·‹ð(9?¢?U\ï=?¥áäªò®õ?îÂi2¸RÜ?Žÿ7´pT?fìË
§z?`÷åù"d?¢j &¹mÃ?–±'¥~ƒ?ê®
FºyŽ?¡åYûiR?'ªªp"?s!öŸÙû?Ä*'ûšÁ?¡åA2±JiAGN4FGL J1456.0+5051?ÇnPtÓx@LG¾ýqÀ;n=þhPÀ<œVœÄÇE@ ÿ‰ þ@Â%ĵ§?Ç;«&ß½À¿§°ÉáàÛ"?ä¾4^'J@JT·è9¿ïý»íx;?ïþ
A¢a¿¿ãARz÷#¿ä81¿ë'á¿ã¦">eìC¿¸,+×õAGNbllRGB J1456+508?ïÄT^ø?p¨boé¬?J«÷3YÜ??¨½nÆ4?zœÖҗŒƒ?oœ}æ<	ô?ïjRü?zº{ÿdV?d\YÈC1?pü,ª ?‰G>œ· ?ˆ
Í`*"?ïfµþCJ?™czØ÷?b/¼	 ?NÏlñHÕ]?ãH³NÖ»?~…ØõŒ¢þ?¡‰'1?…jâù">?€÷æOۃ?i̺ù#º? 4·ïOk"?†I‰Œ?¿Œ¥ô?É'ÕÖ?[çåx¤?PÓEA'™c?ŠTSxÔÑI?
ÝpAM?îɎÊË{?¢5ø ÀHh?r´êŸÇä6?FWâCôM?¡v
!A? a›þÞÖ?îècG¼Æß?ŒQìÜ·¦u?l.÷OZmÎ?cIúAŸ'?Ÿm¸șm?‹æ'†e?ë陞÷ýR?¢Õ‹ÝS£?—ö ±s?‹W¾Ç•D9?ºµ‹Þê?£óŠ?£HAGN4FGL J1457.3-4246?ìGً!0Ò@,¦‹¤ôÀ9'Pi¤ßHÀ;ú²÷8±!@4&Œ[Ãu@A¸œ"Ý?³ïîÿ–gz?¤®
aOG³?ì½7Σf¢@N%zãËí?é-¹a5$$¿ã]Ûèɂ•¿è¡ð€0<¿ä±¾>¶ì¿êhhŸ%Ë?Ëgbû!ôÇAGNbcuPKS J1453-426?ïëÜõr}?Yõ^ü6µ/?;êƒ_X?4´‹rC?`¥º'¢)l?VßôNP°?ïçq S²…?oÓ)3[FU?7Ýö–p2?Eèäø¹B*?e" öE?m/¨–¹ù·?ïoñ¬¢'C?†ßHR鬸?sU&Ô$aä?}"µE›çd?ŠYd^Bc?€S•Õ',?ï÷¼j‡'?3þâCjar?"5üì­?	‡ý¦ò|?OS®t¾x?2Úãö<c?ï݈ÀÈ "?eó»°d;?Gļò¾É?>C_hW?l°Mÿ'?d©Á«Ãª?ﲺ¨e—è?Bîg O?LV¨ÍUÈæ?e jÔÃ9ô?‹ëióŸ,?Ž¾ËÔÀ'I?îÔZ<%d?'Àr¨<jW?€1Y«Ò?ƒ"ß8ï9¦?g(€¡Œ?/Æo¥$H?ïägí"Ûƒ?W Eds?=±@uæ?+Ýt–
ŝ?gáî–!õ0?VUY¼r9AGN4FGL J1457.4-3539¿ïüEŠÆ@4‰"àÀ8(¨(÷À;œÏ¥©r@f'ÿ"Û@fö^–ŽL? )¢].ü?ÅË3²Ù‡@$·ëО¥@ÓH{ÄÇp?Õ/F߸aÜ¿Ýå"ä±oú¿ä•ï ·E&¿åȖÝ&·¿ëwöaÍ¿êO'‰²›ÉAGNFSRQ3FGL J1457.4-3539PKS 1454-354?êñO¥I?ÆXÊ!Ä?­6Žkïæ?±-ôanã?¹ôìaθF?ÁF×)òî?ï€ÜVW¥ƒ? 7ÀÜ_¯?gþNâ©;?y"xĐª?‰ÉV°ÜÜ?žëZ³SÎ?ê9ÓpïÏ?³8ÂWa?¶!fÅña8?§g†Ïvý?¸ý³é^Ð?¬î½"ms?ï܆ýpêµ?á1¨?Rώ̅Û?HڎÑþ8?j;|°è.?Z±ë })ž?èü«¾"?Èâ"r›Üs?ºz©¸?½HSbÊòÏ?½ ‰ð%¹Å?ª&À?îÀMÈà¯?¯eGñD÷?i½«î'?'Hš1Ç? ãnx#j?¬G!+·ã?è\duSä?·L~X¬†µ?¹nàÜ+íø?ª"×8Ç­å?ÁÖý»Š¸´?³ô1Ú\q4?ïg4u06?€ztª?k}4ÏG€?bR}XùÉä?…Æì͙"?|í\®éwAGN4FGL J1457.8-4642¿åé*ó7‰s@%©fàé´À:ôé¦ÙÀ<\E–F_@!¡Í­?ÿ_¥'(^?ÃÄÿa©¿¡I÷šÖ°{?ÛÌsvaÑ@ž™ÔÒÖ?ëUë#Ïèá¿àtÜ?,f?I\ÈWó¿Ú×7‰Úõ¿ç@Z˜ÒÊ=?Ðßn"¤AGNbcuPMN J1457-4642?ïXþ™xŒ"?‹Ö—{Ý$?UX½e¯?H^p"F?"ŽÇVáÑ%?‹;ü?%.?é±o½ìÏ?ÁFñÿ¿ÆÝ?'—4Ñw8<?†x×÷,%?È×Æó;mâ?ÀÎ0¢è«X?îÖcÝR´‹?°ãOT­Ö?k—wWÞº?i*Eëû…? çض¢ÚY?Ž.	]à?íÒ§ç)Q?ŒÄyÂ?u·if[é?]0L>I?°J648z?Œëi^Øq?îG=#L
p? ¿FTâ«<?i\\gÙò?`]úR	Ä?©öhŸXB? <ˆˆ¯yp?âÕE[ƒ?Ê(˜ÿ¯'í?‰Ê`+¦ÜT?"MFE8ã.?ه"Hª=×?ÉÝ€þ?í3'°7Ú|?¡¨ú9á[?wÑ5j¯œ?oÍÕ73ÛÀ?´ò­hû¹l? ƒÜ"§'³?é8€ e"ô?¨S'‡gð?‹n…3j—?{¨eY ?Ég†"i?¨ß!¯.AGN4FGL J1458.6+3722?ä:› @N°hÂa9À:@±gìxdÀ<'¤@¼ˆ²@šD7guZ@§À£Éž?¸¦8ŽfàŠ?«ÎoU®2?ñÀgc¼h@
TœåT¿ê7ž&ò¿Ñ¼J^H¿á‡ÿ¨Â+‰¿ä'Ôôó¿Þ@°ÿç¬L¿ë4o©GhAGNbll3FGL J1458.7+3719B3 1456+375?ïøUª_E?7–?ҒÜT?-4H#ÆÅ?19µpÒ?G\E6å±½?4!H%'ï?ïÞÔñ"[c?o
±»˂??t(Ò
Å$?I$­²%Äw?m<‰ãŒ?jÞmËð?ïÅÿ‹|î?e†x©+×M?U}³•\^?UǐI3ù?w¼›&¹‰˜?a£oš?ïè{<ٝ?F¼x²_® ?HeZ×î?,ÌàØ8"-?aÇ%0Ï N?D:K®áîØ?ïò^¡öàG?H‹2Hò/Â?;#p'N?)'"Ô7n\?Tyàpây?Ec*?ïŸYÑÏãO?"¬êcž{z?Q'(%Ÿâ?ZÌ´ùòIß?…÷fw"ü?'É$ùííÞ?Øo("?s&çÄvœQ?]ÀéýÒ®¯?\¤é>?ƒa,•µ3~?pú¥fžF?ïÀµ|ùü?dž@g
:•?_KDa^?IîL™\à?xe)D-í?bÎTwS±AGN4FGL J1459.0+6129?ì=É9DoF@HÊnÁ~ºñÀ;NéH-–;À<ïóŒT6¹@£À"'Œ@þú¤vln?Ã¥tU·B¿š³ ,Áæ?ÔçñìA[@$»]Ž¦?áú¹¿©Î›¿ã1bV}¿å/áoA¿Ü˜/w便êŸWH¼1t¿ïêøÒU-AGNbcuSDSS J145852.69+612813.8?ïvpöžh?³ëM¬HWd?b+ƒ
ÖuJ?Sp¤Mì¸Ì?Øáå"?³ô"ûxp?ï¼|Nrê?w¿zº•l€?QÔá_ø—?Wå'ÛÝPq?}L¨ ÜHµ?sç³ßgB}?ïM
	n=Ë?"oOQJ˜#?q&7 üm…?p¤•a?'1á…;?3Éåø|?ïŸ2¶>H™?c|7J"o¸?vG Ó(–?X€ó¡Ï¦?z¡ÍÆû?ZíQëšÄB?ïè¦ûŠƒ?¨¤†9?ws*7j´,?j,ð'få?˜† ‰ñ¡?§àJv#{c?ï&$"<Û?•<iÁ#q*?eã mÝó?l?êÕ
-â?˜~ûgý°¾?"	J~Ü?î‹eìÃã?"CŽzJ¬ž?|×ãWXüx?vµßk"f?£®¤ËTfZ?'v)Òâ:?îÝÓ;ÀA?Žÿ²1Pê?B¶xø?v[@K×:?"~	§:ð?z"–nŜ3AGN4FGL J1459.0-5353?è‰ù"Á @Ú\ØH+À9½òJ·À;Y^Sô@§ÔNKg‡@Ն¯²
?ºÒ]Ÿ1Lî?Á$xFÜ?ò͗b‡´•@<Yÿ$㺿ïøe˜º?ïû
H5#¿ãší!*È¿êµg £#0¿å$WÞ8Z¿ä"%B{¦AGNbcuAT20G J145935-535047?í•J	c?¥ŽÌš¤Ö?oq3=Sü?h"2B–?²Y,,õ?¥¶Í;oˆ?ë_ˆÄí?º~€Vã?yÜÍüò·G?€<õ(¯û?Á´³p°AQ?¹U'pW
f?ê˜tã׫M?«©'ٝF¡?¡=Èa¨óq?—Äì|J?ÁNºX0?§×"aåßT?ìOÕ?'äÒîsz?'îv¯x˜?t)6覝?º»™ëñL«?¸ã¿`0J?ëdÔÉy?³+c¬¢?ŽÜïij?ˆKDR?ÁÄ£­¤S?²"nþ†p?äÝÎpw¨?Ǚù2RÚæ?—³™7-š–?¨¤ôÁˆv?ÔÉ)Œà†?Æ
dõ…?ãŸ
;Ò¾ÿ?¶›	õô?³èÓÎS?§fL²'–?ÓÇà€¡.?²ï¨/c¹Ç?æèŸ%ù[?¨Þ$CC[%?§Š
9ÃRø?•Øm\']?Î{\^Ö?¦ÏËVÌAGN4FGL J1459.5+1527?痚»ØˆÃ@M
AÝ!êÀ:ÿ@Iœ+DÀ<œÑ*)Ÿ6@*èãXÕ@Â|ò—?É2.3o?¹y}†8ê?ñ%õ'^éš@p½Úìu4¿ê¼$ô?ï‰ñ Á¬¿ÐÏ(œ¬Hž¿Ü^IA<‹L¿êÙ8¶)ó¿ÔvOýï.¡AGNfsrqMG1 J145921+1526?ïފ,YN?`•X…P*?L¥Ùˆ¼æ??¡ŽªÁ³p?jQª°­ÞP?\yÎz-aó?ïÙíßt£?q÷cɲ÷É?G³GÏrrÊ?RjoyNdV?pz *ãp?moäkÞK?ï~Ø
£?"ǩג>*?n¦ dÐ>e?uÚ!,«?ˆ QÙ6s¢?VW'™?ï¸u¬?\¤n€?e±õ<Îٕ?J—_Z½-?xì6ð8)?U²:0ÁÞ?ï³EîÕ?uSc´!?_
2ãÕ?Q&G¯t?~»¤Ú–?sH5Þ:1?ï‹&Àþ?ˆ"l©…z?Z¿¾+RI?d\³•‡Q?‰ó#ÉiÞ?…bhr2·?ï ÞÎX?Ž6Çò?uQƒúLÂ
?|ÚKâ=ä?–›c"ƒy?ˆ™Ù¦1?ï_»'š	?uŠ,þ?t[eÜÉ´/?`óæ`}ú?ãƒbS£?q¹y#{†éAGN4FGL J1500.7+4752?ëÆGf­è@L¶°hÀ:VL¼q4÷À<Q¶3-Sö@)´½atå@‰‡á
qs?Ä<37
à?ÁƒxǼî?ûúí!*È@|è7"î?áV.	þ‡¿äåܝû(¿âØr‡ÜØ´¿æ- í¶Q¿êÌ_iœý¿ïþ·`Sý®AGNbll3FGL J1500.6+4750TXS 1459+480?îÝ·GÌ¿®?£<[§¹?…iÎã˜å@?{ÛRù+h?™"/™Ã"?‹f»¾
&?ïgÁÛ,6?'Qâ‹~c?€×à."ôÛ?€w§•Q~¬?•§³/TÈ?ˆnsñ¬d©?ï>øìÃì?‰ß؟¿?~=NQ^!â?|³°Õ=?—ÍN¿æ?ƒhrlª?í"ìÛ¶?ˆö€¸<Àý?¢ápÓËÄ?_ ÷I^¬?¤Þ=¬kªß?'•"†Óœ?ìРÁÖú?ª¢|š™ð?ª ©ZL*? Ï\îWþ?±Ñ&K¡Ç™?¢ÙrÁSø?íYs}®µ?¬:â-uó¼?––Xúö‰g?œLYÆ?¯#¬G:4?¢ÞÞR%1?íÂHáŠø?š³x?'
ü<Ýô?‰¯Ý×ÜË?ªÔsĤ³t?""ìC{#?éaB»ŒÀ? ´DG† ?¸?"¬¯Eß?š¶P3Ÿ×?¼¶V~;ð?›y(~Üü[AGN4FGL J1500.9+5528¿Ð+"ÁÐg@J¥éᰉ À:ä¸qËõ6À<¹ªYÛ=©@oœÅóë@qޟ]'ù?Å06(°ù?ÂA!"µ?üê®ñð@#zÉIàt¿ïôL7å?ï¥~ª*
–¿ß—ºò.Ü¿ÜÕR'XàA¿ëó×"f1b¿Ó$e$œíaAGNbllFIRST J150106.2+552750?ïsõ"•À5?~öQ×Ï?tlâ>ÍÅ?kÓÍõÿ9ž?ˆÌ-š¶ÝÊ?{×»Þ}ýC?﯄kEY?€ìÎb¸Ú?`Q?Æfº?h²v¿,¬?€
•>ù(?xõ|~4?îñžŸì'?îojä'ò?{ÔÝ YÍ3?|PJõ"Ä?š×*Ÿ7?ŽCp÷?ïۜ{ÿ³?s•Læ?œøÕ±{L?jþEÔ?CÍ?Œl ÿÃë?l>°OÍ¢}?î¦ÃX"Ña?—dĬ–D?Ž;›nÛÖ?‡ 2¦J ñ?œ
šÏ.?'—uÀ?ﻺš‰ó?˜Ó·ÓGz?v˜Êù Z?|ŸÆ–<@ó?™¡ây˜ƒ€?""s9*?î|•ÁŒ—?Ÿê˜,	³?‡nŒí½û?†Å^93aÞ?©Ü"eä:œ?›n¨¨uí|?íwSôsÛ?'ˆÛ¹?¢ƒ"xWý?…Þw4¸ñ?¤uH`ÅQ?Šd|ZÞsAGN4FGL J1501.0+2238?ïûÚŒ«
@N,ý\·ûÀ9Å㤀À;ýåﳁ¢@úÌx"n?ÿÆ·	)?¨Ì7Tüº?­@
ÿYß<@3Xz™@ÄÓÏöLù?Õcä`è"¿Ûžœ7ً¿Ý©aùDO¿ß¨"í8¿ã
O¿…ç`¿á€`•AGNbll3FGL J1500.9+2238MS 1458.8+2249?ïø@4'G°?Aõz·Â¡ã?("¸ýÚÓm?!;×uì
?HÚ?G	¦ê?=Œ*ú¹Fï?ïÐ:ìÿ¶ô?q"ºô¹ú?HÌs\Ø@ô?P—|®[X?tÈúöüÚ/?míZ®ó®?ï²NI;Ø?xÞéºÛ<?_)@雹Ö?oGD8`l?‹9«±˜?sŽók¦¥ô?ïÆ÷ÍÎÌÏ?WåŸH?_8zâ ¦Û?A<[ÓìÖ?tµú]1¾ÿ?RÞú'L«?ïð¦T×·{?Z"WKËz?9Pµÿ¥tÈ?4)û3{g¤?X_(É;·€?VöNݤß?ïw¼:%?ˆMŸ›g+?`@iär?h¨¦¼ºÜ?Ž*¸¾·† ?…?ñ²ŠV[?ïŒçfx|`?'Y4¶(c&?`&Õñ%?hÀÓKYÙ?ˆ¼pÔÁrX?€'Í•j?ïz¤q
/?sQÌEÔM²?q£m•Ã?YƒÎ(†ú¸?ˆ…-C2™U?o¯KÎ9ÓAGN4FGL J1502.5+5552?®‹ëúó"b@Jo…¸QìÀ:_sN¬5~À<}}Ž¡@…×x¢S'@ú <¶i´?¿0'ùD?Ã=ñÓ'é@ 6^`Þg@P±šÂ?ÏݪÀˆpÒ¿Ýz\9â$¿çEb¹2¼¿ãecœ‡Š£¿çªs;`ÿ¿ïüç|{{¡AGNbcu3FGL J1502.2+5553FIRST J150229.0+555204?ïLcÇÇø?Á#ú—F"?"*4äéB?Àa¼<Yç?jž¢È
~?—@‡Y¦?ïÙÑöŠéÜ?näÊùò¢…?FNv°Ñ×?OPó	~E§?pM5ýbÍÈ?iÙஃ?ïµOÜÐê­?uÞU+ÀB?bSk~%O?pD±Ù)?|.[ëµ±'?m䱂/ûß?ïËuˆ("/?Tæâß4Ž?c϶xÚ×±?AöÃ5D'?p]`¼W'?RGÊò:›6?ïÇáï&qŒ?Jç·¹/+?h™Áàõ?zà†€Ë·
?püŸæIR?e"R2Ÿàì?ïz âÝ
?‹X5'5'i?]Օ?dƒà"f¿&?Ö=佁?ˆú´U:?ïyõ&ÄK?í¼?»Ÿ?q"žlˆ…?y;·ÈŠœ?ˆù³Š±tW?x‹.eT?ïKòÝ‹¿?vüÓh†'?£Ùõèl–?dk°"(;6?‹_'N)¡?s–|#'$šAGN4FGL J1503.3+1651¿æòƝ¢Ž@Lï9C¬ÅÀ;4<ËbÀ<šáìÂo@ îÐ,Ӟ@Ü¢Ûa»?œ{á¢ÇÁ¿¢Ø€'y©?âU/<-­¸@³ch…$˜?ïÜe@Ìxê¿éÈLŸëÃ2¿æõ=Ïng½¿æ±Ï»"–%?ÁuîÚÛz¿âp· gAGNbllNVSS J150316+165116?ïzžsÀc?ƒWä©ö{¢?X[bež"ÿ?ItCÛäM5?ŽLö´Äñ¡?'»ÐH!u?ïN-Ç'`0?"°äO0Ï?pLˆúóG?t¼]$ޅ¬?''%µµ3?@'k'È?ïŽu=·?ˆ
ÛºÌ%O?fëg¦Z,Ô?cÝoÆÝ+?™Äiï
y?‡ƒuöU&?ïZ¨¥{$9?u=?Ý*ßó?WjbA70¯?I-ûÀV¶›?"4E,ã?u	çÖÓ^?îæhY° q?•Ê¢y\ÐJ?i'€@Ïþ?]Ñ!:KL"? bbŒm?•·Z?~«?î~çÚfƒ?¨ªƒDð)?z5÷€ñ÷?‡¡u?¤ÊÃkÑ¿Ž?¤ýU…Æé?îW'¾çy?"\\ªÙe•?pŒ#Q´?h¥ïÃÙ?¨uSPJuc?'àCJx6W?íG}<86ö?™É+•u–²?w‡ño$@?qߘikŒ?´S] õ!?™x…ó€‡þAGN4FGL J1503.5+4759?çý!:Q#@Lx•¿ðExÀ9²amaÚÀ<I핚0˜@ÜB4-@"j㣨ç?²âÚÖ$å=? Èé_Ìæš?ï
	žs`@	4\Ç×­¿áÛÆ«±Ê¿ßێ0¯Ë4¿ä?KâCW¿âyÃ:|Ô¿çhƒweR¿à"¯\y}šAGNbll3FGL J1503.7+4759TXS 1501+481?ïëd²(©?\–Ʀ¦*??2¬Î¨?1Kl»ß"ì?`´øA[J?ZnõœÜª?ïËt¡´è?wÂ½^?M"9ù~ Ç?W¶ôUÍEÿ?v¾'þÀÄ?sØÎbw2?ﺔméy?t¢€Ó7°?WE»ù?cŽcÙ¹Ý@?|ï«<ºáŠ?rgŠÏæ€}?ï ^1'ÿ?cÚËÁ?s3v\Ð%ø?UE'Êên?|q,úr??\'͖û÷?ï×>L/È3?d⮹Ðìx?QŒÞÈgUV?BïL⨗·?oûD^E±î?bOYìôÍ)?ï]I}ˆ¨?#· Zl?bŠz´¨pþ?oÅÆûQòr?'€õN'?‹–A=L?ï–ÌÊ.É?y%ߊ*?_(Ã=åèI?_ÓЌsæ?†š4X©Ê?v´"šM?îù…9:^?'h¬áfè?‹åÔ¦M?süê:]¬S?"EÜn…¬?zÒX?ÆdAGN4FGL J1503.6-6427¿èI‡‹ÉDÀ"{¦iŒÀ9‡B,Ë:&À;w›9¬Éø@äuÚ͖v@¹NþjԊ?ÀÓbDé?ÁŽe³ãó@
žá×öÌ@
¢¸ý0?ïêž‹¥»?ĶúÓpTý¿é°Oô4ã¿â1i.—ÿïøÛH"?ÛmNâçxAGNbcu3FGL J1503.7-6426AT20G J150350-642539?ïM!/òÙH?]Ò)iA?bÒ<ò?aQv$©?"?»9£ü?‹Ã+Uœ©>?ìm×G`M?¶D¾¡Àùh?d'šãkB?nФ}bSJ?»í0ìQ?µË¤†A)?ìr9¹?£¬´þtƙ?"àÅȹ§2?Žà.%Á²?·w""úë?¡êl¸•)?î­|«³^?€7bªÄ`?u:Ï'#¿%?Xi{+óx?¢‡¾OzA?~†æqÈG?îm»&Sž/? €l—ëµ?x[Àss?vÈôÜþv¨?¦#â6°/!?žú5>9òK?çauGWÐ?È)û?ë—,?t­JfË"?Á^Ǜ?Ðê^jeñÄ?Ç°c¤Xÿ?êÆ?šIÂÂ?©¾Rþ£d?›sn˜¬7@?'ö"9Cv*?Áx"ÅDBO?§·
Sý?ëߒ¹Ds'?žYgA±ü?'gU¦ZI?{+ƒ^•FÚ?¼i"̳Õã?œ$í}ÏíAGN4FGL J1503.7-1540¿Ñ
)€E8@B?ÿñÀ9GúËã˜ÁÀ;Þª; g@ ~fpâ–?üLû[V?°ˆà <ó?«ƒÛÂ3?þÓðÈT˜@P†èçày?ïáŸØwü¿¼†ˆb¾¿àÐ^¼>¿ÓÙÔ½\¿Ýt§¼òå¿Öyɺɕ
AGNbll3FGL J1503.7-1540RBS 1457?ï-b[6Sñ?®%]2??hÎê$ö«?ƒYšCT.?—S:Ã(ô?©³êâ8N8?ï¬yîáþ?­ÓñŠ}?`²'̼TÜ?hIã/±Ó?€´ß™xτ?zÒ°Ðc£r?îû¼qéYÿ?o'n^?rfÜ{i|?oG—4äµ?›îº§>'?Šo§£_¥‰?ícp€y@?ƒJ.Y¿m?ð0'	¦t?jèkd!¼?°«ØV/ñç?"¤›)†?îÅé/rÎ?§®š©ª'?q䚟*3¥?w"ðfK5Î?¡dÙ¶y«?¥j›ü¶¤‹?ï0´*<?•)…Šn'?q0	'"«,?w×6š?•±'ÿ§¿?'¡Êå?íïÓ»©d?œºÃ"p¾7?ZuÚÉÏ?~ ¯?¬·¾æ¸¹Î?šÕ¸ŸG?éöµô©8?ž•cÌO›Á?£<[Jàk>?‡¢eŠu?ÃV]å'P?›¹%ìqÚmAGN4FGL J1503.7-5801?èZOׯ?ݦ‹D—3¹À8%ª]6;üÀ:Dã¼ÓZ†@BÞS\ôM@ÔxþŸ3?³ ~Ôá?ÒL''ØÛ@!€¿®Y?ïî‰ÿó–?íœtà|¬ú¿š¿?#49¿ã§ÿT0¿è%d=—:D¿ëê¹FÞ
ã¿éý¿è,AGNbcu3FGL J1503.5-5801WISE J150334.23-580119.2?sŽÑk¤]'?qz5LÔI7?Ùm4üÅ'?ÍÞܪ÷v*?ã"HP"?ÍǐFxy'?†ŸvŠ6T?ŒíuÐö?àNÞ
‰'?Å=½¶ëu@?Þ­Jøi?Äøª§š‹?°oË[[æô?¡‰šù	#'?Ý»'zå›È?´ª¥Q"—?Þ(å­Õvü?´ÿ –óRò?jš-‹O?`V[A`?غ|Y( —?¬ù‡áxdò?ãd–þ'JN?­]dóÀC·?pÒýffG?fÌ×ÎüY…?⛕T?ÉÏÜ"øté?ڈ¾¢_o?É¿A¶ñ?tŸÓ`ÿ2?{9Ðx)d¯?ß8éy̎?É
Ù|')?à:K™—§b?Èù}q'5ï?¢Ó~wí0÷?–@A^{'Â?áZxq€Ì?¹'­$(ë?Ú¢Û@qÎé?¸ÈÙ쐤?`ܗ•@?I4³VÃ?ÜIŽz'Ôj?·ð™ÄWul?áÊ\*ßbã?¸ìÐ؈MIXED4FGL J1503.9-4247?ê"!…FÑ@+k{[À:5âÏòÀ;ý+ÐhbÀ@‡[ÿZ>@O¡—Zû?ȅ#ÖH÷k?Ô©Äõgö‰@^n<ô}@ITݧæ¿ïÿýFKê?ïÿÞý¦ßR¿å€èÈ«ÕÜ¿è>¸c­O¿ïþ³íQ¿îv¹?|AÅAGNbcuPMN J1504-4248?å$­¡?Í`eŽ'ÂÆ?½½¶ò›?½Þb-i3?̎ÀÝª?Ê*Û½?ê£WÈé¾J?¿Dn;iZ?¸	åtøö-?µše¤"\?²Û\BÝ0ƒ?®ë>G¦lB?ænȐR?±m>ŠPç©?´=™r׎?¡]Cêõޒ?Ì)P,ƒ?®[y',?éÁv‰cv?˜è£ƒWÕ?»¸"àÅJ?"é8¼º°?¶;¸£™#‡?‹îÅ)œ.ë?Ý#À'S?ÊsºëVƒ?ÏMdÂw^[?Ěñ¨¤N~?Ó?)ÞB7?ÊÎ$Ô´M?äE¡eÑý?È6ގk=;?ËÎJñjæÔ?Ä.›(ºß:?Ã/wM$²?¹Švã	šÌ?áiîsCL?¶hé`·?Â\†‹?§õb°2ê?Ô#\ôÖ3Ü?³yµûœes?ãKê=ÇM?«ŒëÉ,ÓI?Ì#DŒ»©~?©¶ä+
—?Æ­}9P?¢Úzj—]AGN4FGL J1504.4+1029?Øb˜)_¨@KJ¥ß"9çÀ6Uü6GÀ:ð·E|@á9Q/r‰@þÆDƒ?€OH¬[?¹>àæ_E
@1`m?ž{@#MG0– ¿ÅiÌLtM¿ßzûÿjXä¿ämÂæ™ým¿ägHÐöR¿é:®ƒ¿ëŠ7KšAGNFSRQ3FGL J1504.4+1029PKS 1502+106?ï‡-.v`?Œóäe[(º?qÇe¸ù&¹?x§ÿ†³
ø?…Q	7(³?…™aDÑ[Ì?îX—öxº?·??g~QZ?"6˜ÿ|Ê?¬Òñür‡? [4ÚsF?«Â;ÊíŠÄ?îFI¹Ã–Ô?¢wÂaíc?žë[å Y&?š`­_Œ<?˜Klç"6I?˜x¥G¤'?¯aç?ŒÑw4šÉ?~ýuŒÎí?'úùMæÀ!?|Á2¼u#´?xØÂTîí?î¡éÑ.J/?¤Ù¡"ÏÃ?{f%"]Fa?~â,SDÉ|?¢tž7ŽÇ?£ ¯Pyºã?ìSË?Å
•@³?¬YÉS~SÙ?ÀÒ*"Á,I?®u…«4¨}?±Ú~üøH-?î'~ïìƒï? ï*n^?"¤Þn¹0?•‹wô¬…?™ $Èú?—˜T5cz?î¬ù
P(??¡ÉQ
ã?'IEM¤éþ?"Ѷ³´6¤?˜™ž@"?–.âl؈AGN4FGL J1504.9+2027¿íEeh ¹…@Miáâއ	À:'èYñ
À<q¾7Ô
@•)h¯@¼l}ܟ?º8yÄ<¿£Š~•?åtU!š"{@ñm@U¿æ°,X¿ã8Zðž´¿çu\}ÚKf¿áÕë#Ïèá¿ãކžR¿ïÝ€ÙYAGNbcuNVSS J150503+202811?ï¬Ìe¸…\?˜c‰ëW2?T,ƒ"(-Ï?Aû)"{·?'GV%Y?˜dŸÝm"]?ïÂRALô?w&ܤºkÃ?LX"°^	?R:Ii›7?{Kã[l%Û?tøºjåF)?ïj=ü\T?€Íý^‰?gM%CѦÿ?`á–IF?§'$EÕX?}ú'jÌõ?ïd›¨?m
^L—Um?rðUHy?V"²øßQ?€K‡²?hï¾&kb?ïO|7‰?ýnnñÆ?e›uråÿ?T/Dï¦Ê?"|HûÇa(?/xðUÜ?ï@é{ür#?'W~c£œ?a1Åjšâ÷?eP6$œp?•¼—ÓúF5?YŠI•V[?îã]÷›Ç5?‰L®?tÙ4ÇÚ`
?g¦ù‡u"ª?ž]óÛlhW?‡#…4?Ÿ>?î%æoœVI?‹vÒÊ[¼?ŒSÚ¿öó?vÚïۈ½?¦zDŠ¹?‡Eòl]e%AGN4FGL J1505.0-3433?ݕkQ‡²@4°•9¸ˆrÀ: ¤¸±À<;2U½¡·@"¨¢J˜@…êZ|MX?À3ˆX(¶?À êæ`G@<9ҍ×@
†AÏß?Þé;'¦†?ïâӟNå@¿ä~IÏÞ¥¿âX»¸¨Rš¿ç
z!¯'J¿ïÿœb¡µÈAGNbll3FGL J1505.0-3432PMN J1505-3432?ïïÐu¬]?L¯DàÆ»?C‡¦'B?9e_ŽGÿ«?V›T7m].?D¬Ð@gSÂ?ïÙÂÞ®Ãð?u6ˆØ¢25?J"Ӑå
?WQ¼¸è÷H?o›ì8,¬-?pƒL<¤å?﷗…´­?q©JP®É?\G?äÚP<?^Ô£xp<?}"¢Á/e–?mYX/Ç»ç?ïŠÜY²¤?e@ö?v9ñ%
=S?WBìée?'[ÐL¿do?_¥{h€n?ïß³>†MŒ?ap­Cø\?ZX §¼.[?Vo󎝴&?c ±>'Œ5?S~¯´ÁD?ïm›íd{?‹ÊzJ?eáKƒ¼Û?r.oƒ‹ZP?Š,F&wZw?‡òÌæü?ï€N`z?%ob"ÞÌ?gŒìUÞõ?jÒ¤Hd×?Š	,Ý*Sk?zdÑ®»l6?îäªÉ"?J]ðÃÆm?Š{P/!¾‡?s™®Óï¬"?–,þ»²H<?wsjp7AGN4FGL J1505.0+0326¿ãÐù=@I!lœ
"À8Ó§óÏpÀ;ìнU¡@;Ò2¸@ê¬azŠ?©ˆa97??¹^èî–v$@`dÄ¥¶Þ@/½É¤¤:¿Ð"h<ªUT¿ãµ´ÂêÌ¿è1¤½º
R¿èšc"åV¿éœ¦š3¿ïÿrܖnlAGNNLSY13FGL J1505.1+0326PKS 1502+036?ïçƒkž£?b±U/q?P
•®¨Þ?K³Âñžì©?`ò±¦<R‰?Z½_ք"?ï¡P¨ö*?‡A_š"l?_´ìüÛî?nIíI›Î?ƒµ8&O.˜?'îgÁK4•?ïx˜I&Sk?ˆFƒì
?o\Ú·Ì(›?yh¦­pq?Š·5?…Ñ.Ú~©8?ïÂ)ÈGÏD?]´ñYŒà?jŠ¯Š§?Qé àsG?q¥Ä4¦0?RQÏ+§ó¬?ﴊ ¤È?…ë7?3&?by[XÔ?b†ä.
?|¯ó,}B?'€÷½`{?îðÔäüÌø?¢(P
Œ?wvV#È9?‡š¯,ù"H?œ…Ä®"ñ?ž"æ‹FF?ï)Z&À?s‹÷ò?p\ñ‰ûÚí?t/YŸÜ'T?–½€ynB?Èñ;&?ïa¼'Z"R?{'"¯-?ês"ŠÛ£?p†¨SZæ?…¦'"Ì-É?p¨½¤"ãAGN4FGL J1505.5-8241?éÆO?Ù4À4ú9櫛$À:¡Ñ'¥`wÀ<}kgW'.@ >K¶··'?ÿ¤;~[O²?Âsýiw¾?©/†DA\?é«ù®ro@ïÒÇÄ?Ä4<»Ív?Ë*ž¤›U[¿Ó=Ž >¹Ï¿äXý'«Æ¿Ó˜úìð¯¿ä*[…~AGNbcu3FGL J1504.5-8242WISEA J150525.41-824231.1?ï³OõÙ?u)rµÂ(¶?KÇpŸò1ý?<
kÏDP?o‹{JŸ?t-?÷_®?ïÒÉ_žºÚ?q5Ó°›…®?Cݽ…òӐ?Mö¾º¤¶?t˜œÒ‡Ä?nn‹oP˜
?ïce	ïíä?€¾Ã{""à?aΚ@fn?`;‹NV¿õ?'Y‹~Ò,®?›Ò®ä ?ïh‰éo½?j'*‡?bu© Ýæ'?GR˜ƒQl"? 
 (^V?i˜5Úmn?ïXäè?…#Ó±ÒÒI?e%
XX1?qÇT{
¨?'>Û^À<·?'Z)ÿø?ïxßëb?‰d%Ä_ÀÛ?T³eCà´?`Éï$k?cÛ^Åd!?‡Ò9xÇ¥?îòåf\çs?†á»÷[yu?i¡oCŠ9n?cˆ%«ó§Å?žo%PRr?…¦/¯9 Û?îlSü½''?‡X^
Ù?$?tǼßÈ;¾?b(E(\?¦¡ÈšÁ•j?‡hJù×½AGN4FGL J1506.1+3731?غ"µj@Mó'=[«"À8nd"ÕÀ<3mÖQ@D`%Z@/Þ|·â?Ÿ'†yù—?ºA–{@GՁ§4@Ÿ¶'³y¿§¯Þ™AÊ¿ãÑél?Ä;¿çO'ðßь¿ç¤8#\üZ¿ë=8À:î¿ïþ½	á*RAGNfsrq3FGL J1506.1+3728B2 1504+37?ïʐ3'?sOg"-?fˆjiúžX?`¹'§ùÖá?nçjõ'©?míȏJ;?ァË"?~o¼¾x|?Uè¢%H€?e:ˆÈ¬#?{ý¨~»$4?yúàËx4'?ïM×	¢Ò9?"€¼jý?y?¬Vgò?"l™ÚÔÆÅ?ê´Jg/Ï?¢gg{
ú?ïüjØ¢)F?%"¤l#'ã?)UÖÀFœâ?ÓÂã³O?/ü …ÈÈ=?}÷Ù4l@?ï'Øû._?Š³™Öóo¸?hsìفý?c£±ÿKº?…lÅÿgÏ~?‰DIŽœîì?ïCþ¥ef?™U}¯R?cœT‡0Sa?}¶4Ž‹Ì7?•£Q~Lâ?—uTs}XÏ?îéÓèÂC(?šä_̪y?z¬õö?'¿jŸÂ8Û?œ@}]H¼z?—ñ íuÍ?ïör^°Ì?E;Á¹¡Ùž?@ý‰SÊ®?7£ÁÂÇB"?E:uô5Ä?<恰Q¥AGN4FGL J1506.4-0540?á\˜o"!¾@Eܺ`À;{kà"êçÀ<ž`·Ð¼@"ìr'9Õº?øYÙû‰xº?×\ýç!?Ë©=¦~¯?ñÉa=1¹¶@/ªÁŠ$¿ï')` §¿ïéMcÓ?ï÷3¨£ø˜¿×§amÙ!o¿Ç<ú\Rn¿Ó^U`Y±øAGNbllNVSS J150637-054006?ï«GR5=5?w"‡~œ?S=¸Š²n?EÝø`÷üD?'Æt\âóÄ?vûòš]Ú?ï›å.•s?‡I…‹»m?^>|¹û>?jF¥¨?…>äæJ×}?'ð¼f[RY?îÉÌõ!¯?'œÛ?Æ_?jÿrª**2?t"§ßªb?¡³9†gk?'ñ"'ÎÈE?î…¼Cè?Š	4Bc
'?L&ë† ??CþSnŽ?§=çã›É´?‰ùŠ±N‹?ïCç3?"|ÉcH?cÿr,hw?WÔh6›V?™¾W¶l°z?"¶ß$¡?îök~už4?¦rx¿ð¡?jÊnVRzª?zúã=)Ã?ÙBiŸ"?¤å}ŽDR ?íÌ$Ñp |?›î²y:Ý?sië¦N7?{%òz8Ê?°h:ÆJ]¹?›@ïÀ_°?ë®biʀ?¦}ZS ?U‹áÍË\ƒ?SŸšt(¿?Á^—ÝNG?¦‰Aü‡wAGN4FGL J1506.4+4331¿éøxÞI]@M!ý`éNäÀ;CEћh§À<˜&B‰èL@xU'¾·@¶ŽYÊv±?ÃٙycCF¿§‡¾د?äöóaŒ@ö^KdØG¿Éà ¢6÷?îÁÿiW2¿âg`âC±¿å‹	H~¿â3''d3¿Ü™špY.oAGNbll3FGL J1506.3+4332NVSS J150617+433413?ïÒªnø¯?e=ÐcëT?Qëtê9ª?C~:²²§?r/ì—ž#?cW~wi€?ïÌPcçþ?r	éŒÅÑ~?Lt"Áæ"L?Qƒ|è"'?voÅHÀc?n#-/yÇm?ïOAŸe>&?ƒòzô¤jv?mïZ‹ÿ·?qÁó)«¾–?'YàÆÿ®L?€ˆ+†¬H?ï~}Á̾Š?k›0³0{?n¤eÅ®'?TÊ˶de?ˆ·v´[ã?iÊå9%Ë¢?ï¢Þ¬½Ê?uïõ…eù?f£°;wƒ?_"'nw\y?ŸhðjDò?r">¬Ëì?ïdÿ©äã?Š0¨~Ð{?`Õ&èîÇ?j¼^þX¯?'Ez-y¨?‡s³Ü?îÚk£^‹É?l?w?vð䀳õ?uþš[JÓ?Ÿ+Wž½ê?‰'ålÎ+ê?îk	u O?Œ-e¨Lü?†˜Kž‹‡7?w‰þµiç?£©\³žÎC?ˆ¬TðæðAGN4FGL J1506.6+0813¿èvKŠ±¹@Jl÷ µíÀ9_N"¢Â7À;ÍßgDX@¯T§¢ò?ùŽ%)/?³¥µ%ç?¼<©>'X	@—ƒ>äA^@Û¯fœA¿Ü]ÝÙ¥¿¿…	ꏀf¿ÓþuÜ{ ¿Ô!}Uì¿Ý²ú"¯tÍ¿ÜÞì>Ø
AGNbll3FGL J1506.6+0811PMN J1506+0814?ï÷ÑY	³?=£ðÁ8æò?+.1j™\é?\"©3Æq?IïQj1?:SRæž6??ïÑj8á{Ž?sýíïÆ?KæˆÛô^?Rï¯Ýt+?sÎqm'Â?o´ÍädB?﫼%#"É?v
Å2|—?a%t»·#_?g™KlmB?€Ç™TnÇ?rAÍP
ˆ!?î $Ob
Y?ã›>ä%?m?QNÕ^?L¤ÛéÀkO?¤)Å÷ö"?["ƒêÙ?ïóÒà?I8ÀÒïüø?4˜ªEÛo?$«ãÌp²d?S4uÖ
?F¹áÕÓ?ïz´¾°vÍ?Ži‡JŠç?[놫TŠ?d–§rQÙ?Õ_'|6?Œ'îƱ?ï"HÔ¸²?€•aÄ*?g(œ9V ?lqrɚ—?‰/Æ»<‹ß?|ÛU)"Ô^?ìíÆÖØX5?›)CÁä?z̟¡´]?b5&1Œ²?¶äÿYÎ
Ñ?›!BÙs'AGN4FGL J1507.2+1721¿æ½«Oà¤+@L™£!h0À:‰\qÀ<Wκã–=@ em¿öûu?ø‰Þ¦$ ?Ä/g Ë}?Îæ|¡;N‹@¹A|¢@	ت•yµ¿ï~Å`?ïp?}ÄPý¿©×!~CÁ¿×ŸlAqºW¿Ò`½§?õ¿ç"T¼÷AGNbll3FGL J1507.4+1725NVSS J150716+172103?ïâ8Š!×?hº"k*'?Qê‹f<ý?Tî+;tú™?dÒ¯Æ1Û?`–UnðÄ?ïØ	íй¨?rCœý??FÉþvËö?P« Ëȱ?q!ÉIy·w?n½×¿¤?ï''u5v?Žãw¹Âe?rÞç~lS#?vpšÑ¸Óö?–W÷¹ûz?ŒOž!3n|?ï–ÑúDe?y¤žóÒ[?i• bÁV?Qä@V)X?šš…ƒ¶N?wü‡»ÐÅ
?ïÀO›ž¬~?s[¥<lò7?gF³º¢hÎ?c""Ž‹ƒ?t4Ø_8?k§ˆ³V?ï€÷Q?‰o'šŽõ?\ë‹×̞–?cüc¾˜c?Œ[оÒkÑ?†fhp«'?îl¶eñæ&?™ÁJÚç9?"1ÖR6Í?"'¬óòN?¤($	À5I?–ÉÈ¡Ê°?íÝì~™?"©Á)ânÎ?vh
o$1?f•Ì¹aJ?¯a¸–e?"`!ŒFAGN4FGL J1507.3-3710¿àçTñQš@25ƒƒ­Ÿ
À:_'j@À<L$s|Ï^@̤.Èë@wÖޞ†h?ÂXê§Ôó?ÁG֘Óv	?ýœ¹ßŠ?@W?Ñ&MÈ¿ïÉU^?±?íf.¢<Ö¿è]œ"I¿ÚébÖ#c¿ä%ßøù{'¿ïÿï¿@PAGNbcu3FGL J1507.6-3710NVSS J150720-370903?މÒk?…Ï!Æ?ošHÒëi?u)ƒµa?…vvSï@j?}W!œTVf?ï†h…-.•?ŠPG܆ªß?p{@×ÐOÓ?vb%od?†(>O«jÑ?'4.ïKcÁ?ïIb…Ü#?€‰&aÃj?qÁ­zÈ+Q?o)¹¼1ô?'oHWõ™Ñ?z è¶>î6?îR—v£$?}ztðÂ?" ×ì­?qÍ]î¬?¡Ux5ÿgë?u³Ê9úî?îø+®À®m?'iÄîË?…¾¢:ó‰	?€414J¿?–9O¥Þ?‰ÝLjú—?î®ü@NJ2? ÆñQ•?"÷¬w×Lä?Eï?Ÿ¤¡¥û©c?—X[ª®fq?îq'ûF²Â?'Ì[t>?ƒiO;ð?}#XMŠ©'?¤	eúó¶"?ŽæÔ¡1²b?ëïV³|*?–¸ôôµ?§1âu1ƒ¦?‹î^øôÇ?´ìY(<"?'b§ç{~ðAGN4FGL J1507.3+3341¿êÏú#G-@N·=CÀ;1@À<Ïâù^ü@  ¿þˆ1?ø¸¨RšÈ?Ó­Ü|m8è?Öõ·ý‡Õ¢@f݄ªõ@\[J©q¿ìiþ Õ®¿ïæ»@2u?ï›r·­¿×@>Æå,¿áp¿ïÿ⾦™\AGNbcu87GB 150531.0+334938?¸µh­?|nZAèQ?^¥Äç¬F?P;_o=G?…á@?z›f½3x?ï†A;ùD>?[$ÏÿB|?fÛ\—»Š?p>Ya/*?ˆ¸ÙÞ¾?ŠÌðënª?î¢\:,e}?–f2‰Ì?uæFNxó?y""¹e?£s'ô¾ì?"¨l³Al?î‰^
wRG?ˆ¹Øøµ)?qêÏ¥šÝÕ?`áՒ'é?¥,ÅgËÑ?‡›¾,¹?ï=ü;ò—?#iš³Š?iÅ-i˜; ?cžyÐYè?•#zÆ1¸?Ž´Yþ?î£7zô¢?£šÚ´²rÛ?wÆ)TÃì?€î<Í%Ž5?¢ÓÃ'…ËŸ?¡¨±Ûÿl?í­'§¦|?¡BRlÖºY?{L¯r×2‹?zLy•?/Q?°ßËýbú? ¼œý÷ô
?ìØ.a+,î?¡Ú³¢%ј?v/½ÄY~Q?rA¸ªÖ€É?·Û'(«?¡sÇëð@AGN4FGL J1508.4+7717?ätjžbç@B¬ÜY1ÊÀ:ò¦WíýŸÀ<ã™hò1á@c`í*»@,næg¨†?·ž¹¾þ$¿µÑž~ìÖ>?úáՍe®±@‹Í(<_¿ÔǙœž±±¿èï^¶¿â—À%çñ¿áž2OÞd¥¿áüE°ä9¿Ó9ïô8AGNbcuNVSS J150811+771819?ïëFå9!¬?€F¯ó?3b×g¦?5Z%.‡W?bLڗÇL§?úNC'›?ïâØd'b?kÿ]·K÷?;Œ¤cÛe?GR'?i¶I±‹?fÓË*H›€?ï"V¿²æz?'yÚ^s9q?PR$·Ý¸ì?TçŽÇ¾þ?‰ v^W?'\iÆÊJ?ïë Fö£?G¿Œ0<c?B' T?'+#—g´?`s•áĤ·?FáÑIãÝ?ïß>œüX3?mp+€<}?KÇÓ5	Uñ?F¾²ò.n?iÏndü÷¿?jŽÔšÿ¦»?ï¦wkç?'	‰—G³?Q¬æyãó?[Öz]"º?",¡Pù"é?€
L«ìË?ï&Ô=–?Nçáԅy?^<k!S?h¢å)ÞHg?™E6ŸC?	ÎvJS?ï³Z¾ù‹®?i¥ot"È?_íHjù?M¦8©Š6?~WN1šŽƒ?hKK'"³#AGN4FGL J1508.5-4951¿åã~JïΖ@Ò´|lbÀ8´"}Ðæ7À;; 'oÿl@œY®ê@žÚH¶R?²5Iè‹o?Ō¨Å["P@sœcxu@–,ÞZi?Ø¢@\;•,¿æNI¿ê5`Iô¿éF3 ÁV!¿î 2:ïÿóÖ&ãAGNbcu3FGL J1508.7-4956PMN J1508-4953?ï?gc]ê¹?ïQÙ|ãŸ?ŒÌnH¬?ˆÏë1´$'?ƒY¸Ûa»¶?}g2DZ°?çÍ¢wŽ­?Ç ÁKx,?µ*Bǃja?¶ð¬fÃ?Æ4àrðÛ?ÁS)¦J4µ?ízŒ"‰ Ž?¢rÏΆv¬?¡™Æw3˜R?˜Ò@,ª}Î?¦½p=ž©Ë?šjÓ?êB€š3_?–›K7›S¬?°óڒ9&]?"­NWPõ?¼ø šv°®?s:™µÇm?î\»k?£ø%L2*?¡7®q[ѧ? j·¾N®?'ù@ô	h?vA6p?â‹z:¿Õª?ÐGô"î½k?ÁÑ·WŎÀ?Ã'1·]$?Ò/ޝM?ÊfÁH<ã>?ìMõÕj?¦ŠÐ6»]L?«ýΤ½?¡A­ØÐ?°i—šÒ?œýI¥)ß?á[øÃdˆ?®Û«mô©?ÉûPߧ¬?ªœ×Éwz,?ÐJf	cð?¥Vcñ¹b¯AGN4FGL J1508.8+2708¿ï´š	/@MÄ6~ANÀ: $-ÿîÀ<Rv‰Ê@~ÄN##œ@¦M™æÆs?ºâL¤>Ó¿¢F—'×Ïú?èŽÙ·–Ú¢@5ù¥ž?ïìh ¤Ñ¿ÙãºÚ±çÄ¿åëÍ
dl'¿àSÞ9ۿׯ͸…,¿Ôá,Ö!à%AGNbll3FGL J1508.6+2709RBS 1467?ïo«t*—?ƒŸqÖÏ3?`‰4o'éè?QäûlÈUD?òñ‰ £Ú?Úqŵ?ï‡\ÚeV?ŠãO!#±Î?b›™^˜_?eÛ@æIª?‰žAèæZ~?‡ˆø'JW?ïM¬˜qGã?'[ù.¯?eÆŽü$?aåžh€?"š4G"?M_—ßÂ?ïûó©O?s¹¯Øƒ
ø?|E³1&ë?`_±'wÌ?—ïÚ´jK?rÆ#¹ŽCµ?îݛ'–jæ?–©îðEõC?po&œü·?aÕ¼ˆÒ? bÉË?•š"LÊ%?îãÐÎnk?—Éžè6U?qá}ôx"?t ç j?ŸB­ÖeÈt?•ãn¡^º?îúÏñ?ë	AÕßÜ?q–U1TÊ©?jÒû…£Æ?£íˆe1
¤?T\'õ®¼?ìÆH'_Ã?"Ê5übÒã?—Y\ïmP?""FÂ]?³÷gŠÓ®?'öÕN–AGN4FGL J1509.6-4334?Ý'å—"@)Íl.ýDÀ:êHޖ#À;á•ÊØ@Èý4s¥@¡íý¬i?Ë|,Ñð"?à.Ò`Š"S@})Àµ@n埬ƒ?ï¥(xÅ
¼¿â¤9/Ìvf¿é½¿ÚËé¿é×ñ=Å]m¿ïÿù_|è3?ïg4ø/Q&AGNfsrq2FGL J1508.9-4342PMN J1509-4340?èêdÓá‹?½ËH¾?ÆޔD	+?½)ƒ¥24?¥äˆ¥1{™?ŸW=ì")?历ñK\J?ÇpOFAáT?njkïÎjÃ?¿–ø]i?Â9xK$?¿É'ýÔh?䖫ñ"‰=?²ù˜Õ ?ƌzÚA?®xacãÀ?ÇÕ_©™þ?ªrEÐkS:?ähšs3?«à$Jߎ?ÍGïR™ç?§u¸CìA?ÂT`nC™L? ›ê9–»?á`M¼1°7?ÇAíYà?ØÀhÙeêô?È(Àørñ?±ûî»Üzð?ª¾¨7eH¹?Ö†ÙxÇ?̏qF-$À?ÜΟñސ?̞ïŠÎ
÷?Ë¡U
+?R?ÖBla'7?ۍ "3?µPˆ,l—?ÓPÇíƒÀX?·Êó4¿?Ñ!—c•?²Û‹EFp?Êò|r	ä?«òÙÊãÈÐ?àŒI\jd"?·Ã—ÐÞب?Ñn/²Ê?²¶'¿3ÚMIXED4FGL J1509.7+5556¿çÆÔ\°|@Jo~=ÁÀ:@K!JÓÀ<ŽævÁþ=@ 0@	‹€?û÷.?½iSWjö?ÀD,?Nœ@Z'£S&?üöèˆ?)?î0Sà&ñ±¿æ·'I%E¿Ý2;;•Wk¿Ñ¸䓒ï¿àñ¥"yŸ(¿ë'ž^ÿëAGNbll3FGL J1509.7+5556SBS 1508+561?ﺅÅQXb?v¯	ý^¬à?YóÁðÞ?T¿,rô*?|Y f'«X?sqÎ7|·??îÊ-ôb›‰?™©K¢Ç"ó?ˆÙGÅÁ‰°?‹¾ÒmˆŠ!?šM'ƒ—þ?Q:žüâ?ïQ ƒz•À?'‡ÆÞû;^?pzÎOêˆ?rogåï?'½n^M*e?|f2dZ™?섦\9€™?Þ74?¥S,SÄBþ?ƒ‹ý¢ù+à?±16óãæ:?…Û­Ï×OO?É×C?'£Dׄ'?q6Šø4cC?hŸ>µ™'?†Âˆ6®?~
ä7Ù%?ìÄ® Aòq?²ðÆÅõî?ž""xd¤?¢T«Føg?²9mà³R‹?©£P[ðP?îÅ[äØ1Z?'ËLÒ¾Ò?{ß'1æµ?z6Ã[ñ®? .\ÏWÏF?T{#Ú8?盜öñ8'?£Ãn³?·Û=ºáíå?›"cWd×?Å£íG8E?¡K›çƆAGN4FGL J1509.8-2906¿ïÏ_·
¸@8¹yŠ˜À9'[4<ËÀ;ùÙLJ®@Rü'G—@3n<½€?¸'Þ½?ÁÇp×ÙpI@Š.oKè@®w!I§¿¨ëÂlÕ¿çòÖKÒ¿é0]€c½•¿èœPbîâ¡¿ía¬ÃB
¿ïö¾7ޓŸAGNbcuAT20G J150945-290502?ïàL¶3z£?güH؏b?ZAÃŞ"?W'±­‹À?b'zÔ¥
â?\1V,9c?ï½!gÈû?|Ã(Ã÷q?]>ò©Š8b?eØO6â©?zyœ"t?t7å|?w"?z5%Ï9
?h"t¬P[²?lºo¿¸â"?'Ôw™õ"?uC·RM½ì?ïÊ4Žto?e%m¶?q—Y¹õ?RwmäÐÊÁ?ƒÆ
/=¹?`2`U¼?ïº:.á%0?zh썽Yq?qÚ°Xë?pp ùC©?qÉnp»r?nŒ—1ó2¶?ï;'÷­ºÓ?•¢Fìm?r¸],í{?}]Ãóg?"߉ĸ¡à?'éÏl-]ƒ?ïKËí´Á?‡Ú‰4,é~?t%p~JB?r³»kÁé?'}&8§P?"äNlÌ;j?î›°È'ß?‰Þ¡u[?4`L%€?x:c/ҏ?ØÃd?'Wç{"o¹AGN4FGL J1510.1+5702?àÕt@IªB¿˜0äÀ:¢<g[RÀ<ª4òP@¸ˆå—I@
4˜?½€žöЬU?fmȁúƤ?¨á߯\Ï@ú8õêÓ?å4ªÌÇÄO¿çvÇý°Ž¿ìܽ¹‰y¿å/hۋ¬¿än,Rn¿ïúÎg×®AGNfsrqGB 1508+5714?ïì16?i/Åï:Æ?]¿—?¯;?fÓÒ^¶á?E

*Ñ
?Jê#×kþS?ïÕG@öA?q¸øöžœ×?G¼»¾Çó?P²BFD\¤?rdÈ$q!t?mv¦YÙUÀ?ïMþàŸŠ?Žõe=½ü?c	@íšE'?pÕøׯ	\?"ߟ…‰?©à½Pù?ïé•Ê¤uã?Fq°Ä;?Rƒð´m¬?9ä^U•¼?ZPzAë¬ê??6s0»µ?ïäs}XÎ×?sVBñ†~?föi‹¯U)?qýæÚCõ¥?BXe9üëø?Iù«œ¸G?ï~p•¶­s?Œõ™» ©£?WÚП­îZ?aSbSr	?h€|O!t?Šö (È?ïE©c?Ö
Ý -?hþp'?=?q>º'šò>?šüÉU#;ý?1Q2ðK?ï®ô¸Vѧ?k¯>'H:w?s0tXî¶Þ?cÖ#Ý?uU/lŠ-õ?^ŸEñ‡AGN4FGL J1510.8+7959¿î¶ª'í…@A•¥CñÇXÀ:ßB¶]õÀ<êž…@¿kÅöÅ@Eʯ¼Î?Â(Cg2ê?«
jØf?çù4j¤9@êÓ_Ž¿ç4yð'Î?ïî6¿Yǝ¿çD{û#!m¿Û§˜€|¿â«5£OûÁ¿ìïÐ!ëãAGNbcu3FGL J1512.3+80051RXS J151026.3+795946?ì$\ÊA"Y?ÓªÎ
êy?š´[|ƒ"?²þSîĸ?¸0ïLM?Ï=æCR?ïèøa¦
E?h+$_ʄ¸?5qOñ<‹?C*äŸÏ?dYlň…T?dü½·¥X?ï£xýº!ò?'nNÈ~??UAÖÆ?bÁPm,à?"y…Á
Læ?'éٌö‹?ïøÁ¯"´Ò?0çI˜á©?/ð¤Õg·v?ÀNb¹?Dý¸ìAÈ?-]¤NÅ?íö^váfj?Æ[T[ï6|?^Ã7|?©&7dTÅ?¨k®°/?À§EÝ7†³?ﴞ¸ge?ƒ
3\µJî?J ‡FÿúD?WšEVBw4?.ImH	.?×¬zv¡?ïOLó'x,?þ Éýy8?_ŒÛf~?gñZfûý?""ß|o?Œ¶9ÐjÂë?ïí.ÿ>[}?L­œp†?DFY!¬o?16C±ˆÇÎ?[—^/#Ð?IJKÝÃäAGN4FGL J1510.8-0542¿ÝLMn@Eyùa€M˜À8ؔqÌÀ;"
ɇï@["Ì´@71½è?©°åæyF=?¼¼"Ûw4•@YyámmÂ@P¡ú'+6?–ž=¿Ò¨˜Â¿åÇ#ªÿók¿ç;,%ø¸
¿ê¨¿;ê'Ú¿ãkÀx*´	AGNfsrq3FGL J1510.9-0542PKS 1508-05?ïÈ\
$´H?rÏ¡€%NÎ?Y¡B Ý‡d?Q¨5ø
Ae?ui¨Ûkú?p0Þt
"?ïÂ›?ƒÆ;'È?i£›!eÎ?púÈíFûI?…—6·ßñ?{eÎÈóÍ?î­Gý"]¬?˜0áŸAÏ-?‡u
=î1¨?‰}1qá?žœy¾tÿ¸?''¢¾ã(z?î·á	è«?y³V‡2Ó)?ÕE¨?lݱe¯™?š5S]šñÑ?rçs)ŠîQ?ïQwú8?Ž´G^¨Ö?dÉ­Ô&Aå?_I+nÍûç?"BêTÖ?ŒˆÞ´5Ï?03úX?¢[juCíÎ?ÃïüÁž?ŽÍƒDŸ? œüÑF?ŸFÇûÜΰ?î&~."!ã?žlkf•A?Ž¿'ƒÊDZ?W·5±ž»?¥è<uaã?™Û´à?ì`†<'ù	?˜¾]—a?¦cYéýý?Œ–cx-4Ø?±Ê!'³¹?'—!·"¸AGN4FGL J1511.8-0513¿í¤u4='@E[|þX`À9‡ž ç×À;ò鳍a@ ‡øø#è'?þR@ßÄ V?¼FHcÆùÏ?¨ã^^°¦?íé"89,q@ŸâÈÇ߿Մ'!W¶¿è¥žTê= ¿æ\º:¿Ç᝿C!h¿áà¥â}8:¿Ú}çAB?–AGNbll3FGL J1511.8-0513NVSS J151148-051345?ï¾°³ ¬?jxRÂ	?PÇÆM5Ï?>]H|¢wÔ?|ƒÂªýt«?h)0­tP?ïµ·+о?zÅ¢,Ù[Š?XùA¸ò¦?`	(Lï)Á?næ3€?u{—èò?îù»¯\é)?ŒŸ'Žú'?sNéѪT?qÇP¾3Ú?›õÔoV?Š$7b"ê?íà³jêÉQ?ˆ?D£ÿ?ƒü@əõ‰?g ›béÒ?¬õ¹ë?†I3å/¦(?ï}¼?¥¡)?|7Á˜ªF?bœÅ†O†?Qí jåÅ?‹é¾¨¥XÈ?zaƒ¦.Ò¢?ï ÿ¹´?˜D‹Åým?ok"Jê§Ü?}ؓ
f*Ž?™Î›°…?"ÖëgJD¥?íšà•pXò?!¡ÇWÆO?"U*ú3ž!?}Қ³Q?°žUôôÌ*?šúyG-Ú?ê\«o¸}=?£®—Ti?›
9š¨D?…Qfíüœ?Ã+«
¤C?¢}öÊÓ÷"AGN4FGL J1512.1-2255?ÖWÄû>@=~"î9.À9ÎޑoÀ<!שŸ¡@ 	øF£'?ýü}ÿà?¹‡5híJ?³ŠJq=Yþ?ûmAfҜð?ü=aèRdQ¿ÜŸ9`ô·w¿Ô¿eÛüëy¿åtïËÕV¿Ó'vû	 :¿Ûî›ÿzt¿çǸƅŠïAGNbll3FGL J1512.2-22551RXS J151213.1-225515?ï«Lõ?n?rÇÃÈ÷?TÉ(Þªw?D.3g1"?'"Óœ »F?q+#TÐà*?ïyçLªÓ~?¿™gØqë?qq'  .?|æ®Ö-ÒÙ?ˆÍk m?'®¦bR%?ï&é°!4G?"ƒ|Dö´?w´ÿM]Ü?x¡TˆÌL‰?•5Š?Ma¡?O%?@J?í0ébÀЦ?†â'…ˆž?•Ðïvn<?sÖa,Šˆ?±®.ß>?ƒcq-X˜?ïR¾âº†
?"¶­måJm?i˜œG¡@?Xž?V?'u'‰i?'ÕMî®›?îc(:²?§Ӟ ‡¢?‰Ì \Jf?'à_Œé™?£‡»eeBL? \
á®Êó?îhbfÉÚ÷?•*Þ+î,?Eãӈk?z'xqº…2?¥(`ˋò?'å(öj›?ébà*UF·?Ÿ@Ái«æ?©d‰Š¤?Ž¥í®Òby?Ä]QB_?›5»~cAGN4FGL J1512.2+4704¿ï6×<½J¤@L>}QÀ;6©ðÿ±üÀ<äæíàBË@.KAò¿@\Ôí,¿?ÑqD:íg?³#uÐ玚?ãŒf«/Ä@E<O'²¿àdy¡*]¿æˌ%<Ðk¿æ¦j±N¿ÔyK%BY¿àÐI ]¿ïÿç@ìYZAGNbcuB3 1510+472?ïàoTݹ?\*LQ"L?>ƒv™Š$ª?.ˆ½U&"×?kÀ<Él?Yá6‡?À°?ïÓf{×^C?rݕ¶\Ü?BãCö?Kì÷I¤7E?sðN{rðî?päoD 1Ó?ïz\¯zÎË?zN¿Ê;" ?Z5žør$Ý?J]O§þ'­?Ž" LŒÜ®?yVÉ:?ïÇ0 ̲?Z¶ û-¡d?Pçß#©5?3üúa}àM?x.1Ch¹?Y¼S˶¤¦?ï±^u'd'?xd-ªqÓä?Iòz>1)s?;oÅÕkàÒ?'	:ìYç?w‹ßÚ4+8?ï}OG"=?‰èE=ij?Rî¨aÿ?Z™9xÏÑ
?ŽiaÛvº›?ˆÈMŒ$æê?îûvL§<^?ŠŒŠ"ÌV?c¦."ifd?XӔóÊÂ?žp—û[l?‰þ?êr?ïSi|N
?y·ï©ÉM?cc²Òa?SÚ\Øø?"0Ú~ÁE?yJQþ¿AGN4FGL J1512.2+0202¿æOâiÓ>'@Gý›#ÝTÚÀ8Öu£KÜÀ;ɑÆf>@ÁX';§ ?ÿ~Ö|¨È?ªˆSöø'?Ä'q¤€¨@#'\´5ý@SOÄ +¿Ùw<!™X¿×Du»Cš¿àþ‹ Z›¿â¬×cÿƒÙ¿é']ýa?5¿év%@OvAGNfsrq3FGL J1512.2+0202PKS 1509+022?î·Hqÿÿ?®=À¬?¡4Ÿða?­Ç/FB?{z&špž?w·ª¤)Æ?쓓%Ê?ºën]ß?¬úþõ–?´@ýy6?©ËÑÜ{%?¥ùÓÀ+à¡?ìD$:°?§Ïø¼™íµ?³ÊÇ6
lË?£¦9a¶Ùd?¤!oHY­h?™ç%ë+o‹?êІ©q˜?›á:+Ÿ?²ÐÙ˵?yüāç±?·jÿ
3K?'®ÖX
'?ím襼?°1ó#­ìþ?®NÚÍyB?¬n‰sÒLÎ?–#å94'ô?'M˜Â·¨¬?çãáãy%u?Èã¼Ñ4Ä?Á`¯~n#?Ä ¡Uz°Ë?¾'çYÒ?µˆ'\fæÇ?ë#T|óµ^?¯7•Zª!z?ºmó½@V¡?ªë›\ ï?¨îзãá?š•'‹¸=?åg¥+?ªC;s[‡ß?Á kB̶Û?¡çInÁ¦>?ÉAR'6?¤ŸA¿ßWAGN4FGL J1512.8-0906?êí&=κ@DËÑ$JbÀ5˜A‰7KÇÀ:k' ÿT	@VP"&ë§@òa|ÚQ?ƒÍ#Ç?¬ƒÖAsE{@'ö«ÿÍ«@!`&	ÿËÄØâ"Äö¿â'\f2d¿æÉÁ/á¿åŲÍÈ¿è2­œ…Ý$¿æð _ñØAGNFSRQ3FGL J1512.8-0906PKS 1510-089?ãd×hN¤?ÜýÛO=ø+?ת ã­íl?ݸ']<ñù?˜ÃÉ~¾Á?³ŽÂ<ÈTº?îûyŒD,¼?§¯$z›˜?'Á1ÁùŸ?•Ö<±7û,?—05ˆËó?žîaHϏ?ëñ4ÅoÁ?¯@ܪj–/?"¾ß¾÷¥?•0¦®ÐÄ?»†¡ç"D?«—Áß%B?ïŒ2œú?~ Ó¥HE?v}w‰€E*?q¤»Ù?´ë#ó?rVéÖÓÍÑ?ëþ_–}Û?Áèt¤}ße?"š¯ÉOÍo?²a-cÝÂ?ºæ\6Ë?À2-j­"?í/Ò8á7?½yV3?—ÆêÈ{Ób?ªš~¢Æ‰ª?°•ž¼õèp?·ãíÑòT?ìo¥¨¬Ã(?ªnꘊ†ô?œ
^¯°)?'jFÚTÖ¹?¸[Ï`È97?¨¯‹
®?î¿Ϲ™È?—Ðᾏ.?Ž72ÎÔH?‰ʚêèÇ?™L¦ðÆÜ?'¬AŽ×AGN4FGL J1512.9-5639?ߐĀD€Z?ðg¡á^TÀ8Ç£è_ÐÀ:ùҍ.#@T͆=,@dÆS6?´Œ4қ?ÇSy9QÛ?@àþ}=C@ÂÌ«êª?ïÿp\‰n¿Ð
,"óŸõ¿ã¤"CÆÿ-¿ß.ß[Å£Ž¿çIú?KÅP¿é·}z"AGNbcu3FGL J1512.8-5639PMN J1512-5640?îëR…¢°ˆ?š]_—ð@'?p˜ê——òŠ?iJ ±â?žot©‹"L?™'x>ÔF×?ìVEïö?Å
]£@®¾?f,º¡è¤Å?"Ö9¥@«g?¼œj¯K\ ?ÄÇúüœ.†?éT?§W??¯äؽ]þj?¦°C·^`?›áÑZÓ?ÅÚ³ì+?¬éKvŠ›±?í(µøŽ¶V?"'hký"º?v·X˸ð‹?]u‹¾8W?µNÚ­BëM?'ƒýX¹]7?íՊ"ª,Ë?¨G<@ØJJ?|ÅbÕ?vas•R|ï?¯&"œXüö?§þ‡ÎÏ?è4+Åoz?ÊèP¥£¬Ý?y+i–Τ?ŒKCuJ°?Ï)Ô#¦"?ʛ6½+o?çØPe76?±öGi|ïŠ?­h]f¬?žÞË'û?ÉZ9CŸ<?¯OBÜ?èý#+Ô?¬MR·:œè?é´ªÅ{?~5ühRC)?Ë¢é)Jk?«Ž™íC¾/AGN4FGL J1513.2-7131?íg¸$búÀ'c"ÀÀ:´Ôˆ'ñÀ<Wi¯Çˆ@"y¦	>˜@š"ÛÍÐ?Ä<yX¦?ÎcÜwµ@	£1…´	‡@«	¼Ad¿Ð(³"í?ïþ'ö ¿ãotâ«}¿àhþ&,"¿éU¯"­¡Ž¿ïÿÊñ*z'AGNbcuPMN J1512-7131?s³‰?›ˆÙÇÐ?xEÍbš?"" ë¤Q¤?~áxÑ."¬?'P°F¯;í?ï×H{ÄÇp?€Ùぴ;'?:a·"$Z?RÎRğ_?rµ¦YS?€,r4/ô?ïÞOù^ó?^i(—â?}C"€é¸?~zÎñsÙï?•³mh(×f?‹PëÚøí9?ïÙý©a–?QÙ¯ïQs?N(cn¸?5‹¢bgÚò?nxʈL.Ë?N"tÖ;—x?ïØÜ¿Lö?ŠÕ'ãG?~ÿv]}?¿ýíêF`?x"+ݯð?x¾û"â³?ï¥oA<œz?›¥í¢Ì?PzÔÎùË?b."}ø±1?""Õ#XUÊ?žÒ@?íä`t	?¡+úÄÜÝ?'$ð&"'k?™
[H?¨¬èAÛ2?š¬!ëéñÁ?ï¢%¥'1'?n\úʾ'?a·´|ëÙ?P$Ä}™n?ƒ2è¥
r²?jÈ)̐‹AGN4FGL J1513.4-3721?Ú '¹¨@1h²ú"¯uÀ:b寺À<O)1Q±£@"®ˆ"
¿@˜säÔ*?¿ÊgþÓw?­¼³Ïû«?ñÞ¦éä5?ûŸ5åÀ¿ïo.áêÁ*?ïì¢À‰Èk¿å»àì>'¿àð™Ã¿ÞËrÅz%¿àpÊ"M‡ÈAGNbcu3FGL J1513.3-37192MASS J15131867-3720114?ï©BZ(ї?p(Ç®,´ ?[ÁÁ¯ûïD?KXËóYç?'71M2–^?mbwî­?ï' #6?Š˜¹6ýI?nÀª!iƒ?uÑfB1ÜO?‡Ç̪4"Ó?øÊÇYs?ïJ¥fg¤:?ƒ%LN7õ~?nI´nz?jõ!/E¬ù?'Ûiø¶{?€d?àĝ?î,¤µØ?}^¼Ž'/½?'ÎñI@×?rZDp?¤N®©j)ç?w·è…Ï¢?ï1>Ýž?"©ÙÅ®?qæEê$?dZXAÎq?•^'Û°Ÿ?'>íÕö·?î'Ç›"!Ž? ]õ‹Fÿ?ƒÂ˜üCf?ˆ{2%€¾?¡ã¤leÂ?škÁ òôí?wÖPY?{ à4ބ?xœWeß?n"Hãzäz?¢ûuèÌ?Žü3æ¹?ë"Ú6†"œ?–'÷+¤¦?¤u/—rLú?Œ²&V¡?¹&–€€0!?"Ì0²´Ï~AGN4FGL J1513.4-0753?é<–OHxÑ@DuáC|V"À;bˆRIxðÀ<‡çQ³Pû@"/c¤• 8?û§+y*Ž?Ò=ðüVþ?±b;^zߚ?ßÈ*[sCD?ö-.vàÜú¿ëBĀx
~?ߧnƒì3D¿ç+m´Z濾9HËö¹¿ïê[ãU¥?ï²Ã×ZÅHAGNbllNVSS J151324-075450?îœìØR^?Á6ÞV•–ˆ?WõP‹Ë;?u¥h¥?¥~ƭċð?À¨"Ûz ?îãQ«ï1§?ª!{Xn‰©?‰‰®(¢ð?¡C	ÜK¶?–Ðót—±¬?—¢ø|£Ë"?î,fE.]a?™ÜÓÄÒq@?ƒÊªM8õl?ƒuäãîO?¨Fñgƒ˜?˜,Ԏ&É?ì"I§z(?½ÈÓÔ?•‹éHµO?"GÍ9;?¶òJK,î?š#5z]é?îÏ\¡Á†H?¢Ë4ªm,?Pʓýšje?Tv'…2—?¢ƒáBòæ3?¢¿ëåW7?íg€BÖ?µdíßÛ·?˜_Ì´Èô?¨šƒFÃt9?­X>ö¦?¬2§§àj?í@*	
b?£[l£œpÇ?…,©´ÍZD?'þ^r'¥¡?´ˆiy‹õ&?¢€Y¢¿¥?ç´¦ ¡Ç?³êßAbƒª?§<Ô¤#?¢Ê8Ff˜?ÍÕø`Š•?²a¬	G{AGN4FGL J1513.4-3231¿¹O•[ÊÀ©@5r›ÏÔ¿
À9v)a"YÇÀ;¼GÜ7£Û@ÛQv?Lq@á#ôÑÏ?µÀÈ\¥?Á•T{ç@ Öoþ@û0$
 j¿×9Fr«G¿åSFÎñj;¿ä›Âhż7¿çè0Àè#¿é{'{;
¿ïÿû˜'2AGNfsrq3FGL J1513.5-3233PKS 1510-324?ï鋔ž20?U›T+f»??LA"2Ê¢l?B$|~ב?^Ȫ|­à?PÛS¸Ê^?ïâ¨ÙJ!?n.iy[+?D?µ±U¦?U©8¾ýr,?hG9zu$?gQµ}›yR?ï‹)2¬&?= ØIÑ?iˆÅÜL­g?r0ŸÎõ˜‰?†ÓûJí?|Ã6î?ïÃv­‡(?Y+׸MåÂ?I
z2D)f?.ñ<»æÏf?{"ú(?,B?Ww~&ž1?ïÌ< ˜@?i'^^™	D?b#‹V%º?YÚÞÐàΧ?pÐ*¿™O?cl½Ão?ïžDC{Õ¹?ˆ!Ì,DÖ?ZR×ú¤?i×V`å–?…$"0o?"ƒjCšÓc?ïDºnI}?ˆ¹…ÈÒ"?xÑܜDº?ymŸÛr?'4;rè?ƒý—¢?ïV¿Á?yº>·]?aÌ©ô«+?KsWû¬ß
?"rÁ«•÷?x®¯"¦j`AGN4FGL J1514.4-7719¿íu#2¥À0¥Ì·ÔDÀ;ǀ¾/À<àÔfõŸ@"á%T"l?ú)'jÑ/2?Ñ°Ëdlç	?Ħ–—±?ó¥@Ìxé÷@åÕÑ-Yª?ÉðXC=—¿ïÃh4œ¿¿?ïëÇkcü?ÛCå½´€ü¿îHFøã?獨eÓAGNbcu1RXS J151448.8-772249?ï½ Nar?tG°'¼è?L÷ûòýª?B,ƒ×¶¼?}ÙMVÿz?sÕ×ß6É?ïR-è׫‰?©Y[ÑbÝ?d%ü¯¹¤¦?s8'óFÖ?"5ƒRVû??¨¸G‰ËS"?î°1?VñÃ?•'Êièsi?tàK®ûè±?x?sº7?¢`â—/5?"pMß ©?îϳ•iÔ?‰Ý~ß-?^óœúŠÝ?R>¿?`?¢
)½¡]I?‰¦tã°Ê?ï|߅ûÆÏ?Š»PüÜYê?ZE
<éK?R"AI÷œæ?|؅Í?‰ÑB_'Ž?î~Ž+Yþ'?¶"ÊzR¥–?ps¥ÐôΘ?'
›êAÕË?¦¨
¡?µØ&Í«6S?îNòºI?–"÷¸­'?s,"»ï?ut)ƒ>?¨»‹IZý?•éÔ}Aàz?ìO5¶m?©½*WíQÓ?xŽÐTá?}T±8é&?»ýeJKl?©È£è	AGN4FGL J1514.6-2044¿ïÒ÷ޕÄo@>å.rÚ0À:uÜ£¥§À<Ný&g@ìF±ë@ ¿þˆ1?Ã)Wɱ?³Ÿ™/Ò?ñ*¸¾«¢@25¯O>?ïÿŒÝÉtS¿ÝÀÆCÆ©G¿á$gRõpZ¿ãšÍv?ø¿ä;_‡O:¿â"«äøêAGNbcuPMN J1514-2043?陼™6È>?ˆ&ƒ¥ÑM?Gõä2AE?<+ÂHü?ê?ƒžûyü¤å?‡ËŠæ¦?ïÃW±ÓÞJ?rs•~Ïå@?Qyܳ÷H3?S',Փ?yõ¯àÓøå?oAÔ®ç?ïY/¬:?‹ëb	›?],[µ«Ç?^uÕoâ©Á?"LÄ
gp?Š3´×Es?ï7çaðØ<?lÍÒÏ!é?màjEg??IQ«™§?•GØçŒ?kz1'Ìîø?ïlI4&x:?ŠýAǑÊ?VÐ#­§î?PxÛǗº?'	×IqpØ?ŠcF::Ó?ïbߧV+í?‰Â
2ê?`qÜí¨xÓ?c¾gœ?'•Ïw±nK?‡ÈÛv\ƒ?îåþzÕðH?"ý¶hv$ä?gš"ç÷?fL¢_+Ú²? &p؃Ž?"]'±"o?í½uì7È?ŠËû÷þ?ƒ0Í°&Ù?f
tôƒÖ?¯\mͺ'Ë?‰{ó@~ö*AGN4FGL J1514.7-3617?îuMÒpУ@2)•þÚfÀ9ñâ,°b3À<ßMØÐç@1gIp@e›Ã?…Q?¹ì6Ÿþ8?Ï›À:m9@;òá3Œ@©›''3?ïàÏ6iI¿ÝóæÐ_~¿ã9 ²ýï¿æTF›œS¿êjáj)¿ïûÊYêWAGNbcu3FGL J1514.8-3623PMN J1514-3617?ïV#ØÍ6)?‹gu÷d«?ŠÚÑ|Æ
?…0BÔ@'›?:
òK×X?rU"âO5]?ä%ë?†/¿z·ñ?j\"ÙÕï—?pÆhœY?ƒ†¡Ã'h??€t°†é\?î3Žïç?œHa­>óù?¡?–³+¬?–Ò–®?—ôº|"$?ŽX4cMÆ÷?îçT*­0X?w2[¢2q?‰™üp€f?hÂòÝpq¢?–H|wsÉ?rÁ:Ig?î™òãj|?¢%žƒÖg?¥R|$˜Ú?#'³‰k	?'GÉX©-n?‡GoÃ@ãÉ?îÔ!?ô?`? ¥SV×6º?ƒŽÜP÷2?Ž1:oÓÓ?›´iÑa?˜	HLù?럠'&ûº?ª½mbÈÂ?µI€¢]Õ¢?¥÷Kz¢"‡?«rõ©°€?œcªÍ³!Œ?읡=ÒÉf?"rôQ;ªþ?¤£Y™?‡Â2"å?°ÁI‹å&
?ŽíÞùAGN4FGL J1514.8-4748?íÑ]'ì³@ Ü˞Ïc€À8ñOäCá×À;y´{/P@ÔT¥sÂo@M/ãóYÿ?­á©þ–žh?º">eìC
@
~BZîc @xŽëád?Ýw€À政â,'à°«¿äS0¿äÕð'3¡m¿èÄ]'"ƒ¹¿ç ¿B Ž€AGNfsrq3FGL J1514.5-4750PMN J1514-4748?îYš¢G
?«'Qæ@€?eÀäŠïã?h¡×҂?©
Tž'Ý?ª>fYZ¢)?ï??§¥˜?›‰Þ?ÚÄ.?Y~ÐÈwê?f¢Y]s¶w?–€1aΆs?šX'¸k ?ïNìíSªø?†>܋f
?jºëaÚõ?if©s~—S?'Ëáì7¯?ƒ¿gî؎˜?ïo:]€?sõðu\??u¥eYêå¹?RÑ65™?š(¿otµ'?q␧"H7?긲"ù]
?½ÛAY¼‰ß?yÊÓÆa³Ú?xŠ*µž?ÄNß
c;?¼ê6ïD4Ò?íêW&­hÙ?² ÍYSr2?q j‡`?~2'ã•»¼?¯7ɔåÓû?±"û€+˜ç?ïx¨Ø?€`Ä[§?vYñ;Ø¥s?y²dՎZ«?š:ƒšºè?¼•™›!M?큼R9ç?‡?¤Û—?eÍJM?q@ïÖ\"?°Qòœ,Uz?Ž'fÛöAGN4FGL J1514.8-0949?è*ßã¼@C¢õ˜ñÀ8äŸM7ÁÀ;;Ò\XÆk@RgÈOƒ@aC?º"ÄÐÿâN?Ä?ðEwÙU@(»ÆKç@ƒá…Ói¿é¥Ï½—ûŠ¿äžæ.CŠ¿ã؎¡îÒ±¿ãÇÏ7
XI¿è˜Ï¤îar¿ê2ßP]¦AGNbcuPMN J1514-0948?ïæ|í±…?`çðÄjª?Q…ΧÀ"K?UÍÉ«"ïÇ?`ÁÌ,¡C?Sùû2S¢ß?ïãÌY4z?ja?ÍUÌÑ?=³7ýš&?HkL+ÙA,?hÁ;‰ß?e«•@€»?ýä¿)?™¸MùWü3?'^:!~ÊÊ?†çÊ1Å}?žùƒ.á#x?•¨–Cö:?﬉JìãC?g¤"º0å?Bߍ^†7F?.ÆÖ9ò7ë?ƒ¯´cv~V?g}7.Š?ïÏ®œ"§›?pÆDHé?aQM)È^%?^Z2ø3?ou\?g¦þp?ïž!ø õ?…zõ¡~×?Oý)T`?\"ÏÈš?†w¯pÛÅ?"Ô¥ò?íþŒ:Ä?¡55x¦Ý?=
6%TC?•Xhã?§ø¹e–ü"?œ¥ÕÊ0í?«\1?‡Ëã~ü©?\)ÓÚ¦^?PM>id}?›®xy~?‡ìG®˜ÄAGN4FGL J1516.1+4351¿ïi.¤S@L?ނ׶5À:ÉOµò–À<iàš	+"@É´¨"²z?üO§r 0?àxïÕæQ?ægë×TL?ý`« ªšs@…çë·¹¿ë~ê÷Z?¿äöHñá¿áº cÏ¿èΦ´4P¿ïÿšêÒqQ?ïú6È)¨AGNbll87GB 151444.4+440102?ï­Í;:FV?ƒoÚlÁ?g«÷É\v??k*^4«
Î?}Cft²-?~Ø$Ë硜?ï5–'ô¬?›¹¢‹v9o?z.dºeQ?†«Ã#
U?'Æ" ¬Áì?"}vœk:t?íà*ƎU?Ÿe@1Ú~Í?—…¶ê‹š@?"5oàÿ?¦:x#Œ¨ï?—-)F÷?ï<­ì?€Ç-ë9Ž0?d¥"øÅÏ?U¯ÕPµ?•ékC8òŒ?¼àÚl×?ïO®ÚQ"e?•*jÅ,?€±\Ú"­?"À`OBÏ?‹bì˜Ëç•?†Ÿ¤0?íö]48–Ê?¶'@€Ìä¸?Ž‡
|®òß?§Ì,ݼZÐ?¨øj&½¡?¯a'3|UÒ?ìÉè«ÇæÖ?¢ÍL‡>¹~?œŠ"ˆ"i[?"½oF:Ë#?²Ž}'mz?Ÿ7G§ÏáV?í½ìàq"? CS'©Yc?pVœ_ÂÁZ?tL«í¾"?±Ñiy?Ÿ\W°sAGN4FGL J1516.5+0015?Épxg^¢¼@G}$
=À:$í`Á
øÀ<6ðÊØÖÆ@ª4†O@ßöZdÐd?ÀFý•lŽI?²À´æ| b?ñ §". @ÄÓ6Hfv?ïÿÿÊPË¿ã»l‡è—.¿æ‡Í‰‹.¿êT
¾ÊÖ}¿è'vYùpš¿ïýHàÄ{pAGNrdgPKS 1514+00?ï‡i^ÔÄ? `yŽŸ?bç¸:`zq?ˆX*\¡ â?‰k­Îq?˜[p»•G?ï®~mÅ<?{–'Eoó?]vßM_†²?`j@«ß?€±ˆÙñä
?u—íßü[Y?îÿ¸àU?ÓÏBÓ!?q>5Ê®á?sq%{‰i?›Ì{x";³?ìÁ¡Úâ?ï$•`¤Ûl?rœ'ø»À?"¥-ßQؼ?eÝ*ª±?'½šÞ?j§ÐŸX`?ï0rIQ5Z?"P<Ô'Ò/?q_4'"<?w
ÓhÖVÜ?•™ò"@?'ã€Ó^"?ïºàø9?—ÍèÚD~?qžB‡¤M¡?tÐÙbŽ•Ý?›Dc-ã?•F4)ÃÁã?íúùÑ!?š'…‡Ý½?"•…&´¹t?€qÒPÕe?«+'‰Q?˜R¾"XÁm?ížaý¶?Ž¦·'ä?œtª+J!/?'¥÷b?§ß‹½Û?†¨Û€ï©œAGN4FGL J1516.8+2918?š7‰üGÙ@M©'Dé>À:Òwú øÀ<‡Ó*´ßp@ò_­Ád@¯œ'r^?¾` |È念Ëœ¡
ý?÷ÑÓíR~R@?¾VèD?ã	Ñäç¡¿ÝQò;_¿èÝ۝ ~¿âfÚ_\†ê¿ïátú}à?ïw¹_‡¤úAGNbllRGB J1516+293?ïSö57* ?®†Ù«‡?iäÞ<A?ecG&Ÿñá?'D·dç¨t?®O'eÁ?ïyàµÑ¢c?Ž Ã\9?n½ä{Žòo?€œÒ×{n
?‰ØYe$†˜?ƒE¥í`#U?îí»KSÄ?'mUL¶3?uvGQÇ¡«?u
\z?œë:ìq?'8ù" Ðý?ï…iäu5?nÕ1ڟr?uÀƒÈ1í?_V¸«Ó?""¦'pL?f.o0 @?îýÊñ#]?šG"L‡ÍQ?|ó˜fßJ7?uµì;Ð+?™	Ø"]Ë?—/ÁxU³-?CW(í? ^DèiÔ?yq
›Š?ƒ™"Éot~?¡Š‹3Ð<?šþ­*×*Z?íµ¢ÜŽ`Ö? xúŠ¼'?"0çëÂto?'')€Õ?¯™˜8¾"?ŸôÆk'Ï?îŒçtÊ?"{Ù÷?"ë†Zýœ?ƒ•ú %?¤q§Ì³"?‹ý"¬)EAGN4FGL J1516.8+3651¿ïíh ÿ@Lñ¾ne8À;"ªLÀ<Ò6/fö@³B§'@
ª]6;ü?Ä˝bQý?·x°ëŶX?ì®Ö™íý@æ]êÁÕM?ÞU?bžÎ¿áåÓ)Þ ¿ÍU*˜ë¿êo¼árKL¿ßœ_Ý
\¥¿×¡CœŒéAGNbll3FGL J1516.7+3648MG2 J151646+3650?ïí0ù¶Õ?lŠ
*À¼?,½K%{@?-Qᝣn?`¤ú—{÷?k]"´n8?ïÕ¢ N<?pK‡'µ»Z?CÔEØi?Na"I}Ã?r´gQ¦|?lPLƒo@j?ï5õòðM?'Zxóƒ[?`Vãc'Æ?k™ ó¡•?—6€\Á'ü?Üٞè!?ïß!d9÷"?KɔڎÜ*?CƒÅl²k?)yiÁ¼z÷?kýשn&»?Jbå$»3?ïÍ/Üo4Ê?†ÄæEça?AµÓv.Ï?Iޗ;Ç×À?w1WFQÛ?…§`ï"}?ïfµQíÙ?äÚ;ž‡W?RP9‹v¿?YÖúñõ?'R'Ȥ}?™ÙEÜ!6?î–÷vL@(?œØôž.?h\õ1ñmÚ?o1£ÖC?¥
¹Jò"?œkFE"Ž?ï'Bf>Ø?qԍ·ÁSn?Y6Ÿcë?Hšª*Sm?ˆH'—§?qH‹CDj?AGN4FGL J1516.9+1934¿ïK`Ô+:ì@Kð®Bž
BÀ:l3¹jðÀ<]úꉯ@HnÃ>Ú@WC³³÷?½êmœ™ì?oÌ]Ûþ?°¼0Gpó@q[$=÷Ý?ä³½œ®!¿×ö[üÕþû¿ëʝþ-B¿áâ™Ýâí¿âA&»×¿ïõ
8h&ZAGNbll3FGL J1516.9+1926PKS 1514+197?ïðåíy?[{°Ã£?;·$©^‡?=}	µ‹®?Wq^ë¾Û?UM±ãÊ»?ïٜ' K?uZEc¢?@F°ÈLû²?Ki#WG?q) 'I&»?s¿žu?ïŽ75Ó?ØÈÃ"¶?ajZŸ…WH?nÚuín?ˆ ۜè;e?%çèп?ïãϐK'%?JY™¥^C	?HŽº¸Y@?0
yÔS¤µ?fë"ø"¨?Fw›6	£Ù?ïê½8/Fj?]Àž>±ü?DýX©Z<:?@›?É0?`q¸Ð
?XÉVL;?ï"kNzó?—BBæFªæ?P'‰µ+ó?Züw‹¯ý…?ŒÔÛ7ieÚ?–Ô¥5
Ó?ï=Aú?‰ª}­Úã?iîö¨Ë^?méMHI¦*?•:¹ùÜ0Š?‡mJ‰¥«'?禍œ¿Í?g€ê]ª
?dô©Ïž°?R_+‰Ø\?€^.kó£?cîÔm¼"AGN4FGL J1517.0+2639¿îâÙøj›@LÒÂ&€IÀ:¦7åI›UÀ<éᰉ @fâæi«ë@ü¨"1¡?Àæ'w2?˜hͧpÐU?×ւN8ó@«Çæ2)¿çsø`îW¿ÙJzAå}ž¿èxDµ;·¿Øñ±ž6ó¿åTˆM@ûs¿ðAGNbcu3FGL J1517.0+2637SDSS J151702.59+263858.7?ïìòb?RaÕNº?C#
(Ò)?7ýR(?]^	ÞßÈ?M°1ªn*Õ?ïÛÁ‡I_ð?r7,^Ò!6?Aȅ·€Œ?L¦­ƒh¿?oÌWeþEÅ?p,ùÔ?ï¯Õ†Àà?vý'Ìt?Uû–Å"ÿ?T£9³ƒ?R&êUÃß?t`£¹Åy?ïÅßêz¡v?Všù½Û?Xé¹Y·Þ'?9C‰¹3wž?v՜[Ã-½?TßcÒ1A?ïÖd]¢y?gN»ô;<?P‰"ƅ?CnF¬VþN?pÉîºuÎ?e"°ŸR'?ï‰J̬ì]?¿ýVc2?QmìG‹F?ZùáE¾DÜ?‹^*£Z?2¡ÍjŽ?ïqê)÷"?|[–s`½?aIV‹Öü?`BޓÌ?3÷sæ?zcîD÷?å?ïSBô‹?wJßd'º?sI\Ú¿[M?\$,™^àß?Í eÃVÁ?tKÉð$AGN4FGL J1517.3+6630¿ïA &"+Ò@FZý›¡²À;BŸÿå(
À<ÏèYmZ@̘×ÒºM?ÿJBÉ©+Þ?ÙÚ €a?Úڐڮ6à@u4½vît@^ðù²?âÊ¡¿,ü
?ê{|½ë³m¿ãøÄL0Z¿ç·¡Aƒ­õ¿ïþÁU F¿ìÿ8?®ŠAGNbcu87GB 151628.7+663843?ï±S\ssj?upÃÑx?dFrōDú?[Ë_ͳ»?}3]P\t?qcÜ%^Ï
?:x÷¹?‡wŠ!Â͎?lpâìuëß?sÅÖ±x™?…58Ÿmhð?.+z?ÖÂ?îޙÎr¿:?'WüVî?"…2þ[Åa?'ÜþU
Ý?™ê,©ã0?^Nñ¨ïæ?ï1¢8hk?u¥BFWòj?…°À'ÒÑ?nR/É+Ž?æ±í{؎?jUºÍhú{?ï7©ÑŽí2?ˆû$ˆ|d?{âëN'`?ut‡D
$?'
ý0®#?ƒÿË%Ïf?îÇkâ–@?¡úD?¥%?ª?'l™k?Œ¸»ðdÃ?Ÿ(ê§¢?™ت©öÚ?îc»µ¼ÿ"?"a¼î?ˆØx|"yo?"¸SRY?£Ž&"/Ae?´k-Õ¹ ?îfØ(lýý?ŒRݲ?E+ž[?'mž¾=?¢A-l²¡?…é=ŽwÿAGN4FGL J1517.7-2422?Ç%…'‹€@;"ŸDÔEgÀ7o¡vݬïÀ;$óMj@ËBÎܜy@¢U°5½Q?")A9R©h?#59GÊD@À"<jêZ@eŸ±aâ?™—ÿ)‰¿ßGà~ÛRL¿âÛ­p3T¿à¾Q	¿¿äæ
`:Ó;¿à˜ÖšíWAGNbll3FGL J1517.6-2422AP Librae?ïë£Æ)€¾?r"åB†Û?0Ç1JÀ÷?9[
·"YX?bCSŠ>No?qj±Šã/?ï¬æ™ì>œ?"žcZ?[zdÕ
?dR7çï.I?W⤋I?'!î£	ý?ï1;Ó7B?"e!¶ÁÅ?0/¥æ€?†¢;Ž't?'Œ}w0*?üì™(­	?ï±^EzÖ?h4y¡Ý?Z¯¹"2ö?C@ {•`?€RœÐõÂ5?f‹1M;†?ïΤĬ(?w"xĐª?H{;ðrAÕ?p…rñ]æ?uéF,´;?o5'\YÂ?ï/À×Ãm?¡;÷½fRo?j˜ß6".?|Ó~Õæu?–ÙÔÂñsú?Ÿå¦±†Õ…?ïQ<€k?—ö'¥ež£?'lׁJ/1?ŠJ·ØLq?•¿l¨O	?":Ç+l":?ïm[¸ÚÊ?€[R«?h‰U}$©?]qn=t?Ž—"Ër†e?~–­CÙgAGN4FGL J1517.7+6525¿Å§¬Ï"à@F²-VÀ9e§Vñ~À<-s?'½@ ®F#û³?û¹9±Êé?«þDZF?°ìȀ6ò@àäJ7\@	ãÔùl"?ïЬU^f¿Ôœˆ Þ¿á,V4¿û-¿Ððú¾øxÍ¿ØlD̸«¿á$¬ó±³AGNbll3FGL J1517.6+65241H 1515+660?ïëþ€Îòl?W§ c–?3CÝ&†÷Ï?(e,Ô¤?a™G'Î?U¯É+¥–?ïÌ–.ø]?uœÄíhwZ?P½%¤?X'­®ýk•?uÚŒXA?pöÌˆ²«?樂ǡiÈ?wÇVQ‹Ý?RZ'¸ËÙH?;-ˆb
?"M{Å[†ê?ws8íîl?ï<"ÖœŒò?lA·ó¾ò?x½7z?V!eÊAÿ•?'@k4ˆF?i¡Í&Ý7?ï×Çsæp?sà+óÿŽ½?D.‹Õé?6ß=,+?q˜À˜zÖ?ssۗßeò?ïOHCªhŽ?'‰ÎòØ)k?epŽw˜c?lŸ:±?"hå´´®ò?Ã|'ÆÈ?ïa'ÙJ£?†
oÉi?\öŒ¢?^#éb³j?'>cÐÐa?…¯4ØÇ#b?îȗðv?‹z"Ã+‹?9ɳv?v¥»s »?§Õ;ë ?‡'YÂÅËAGN4FGL J1518.0-2731?éì©OUcñ@8ü*í"1À8×äŠX³öÀ;ÐÞô@ï_íüGd@E^ÿiØ?§¤yá1L˜?'ô;X¬Ñ?ê?Q"W6@©¹qPON¿"Òæí4v¿ÉŸ0²Os¿âVæáËâl¿Üýð;ø ¿ãRÄþ¢1ï¿Ý%[[ÕAGNbll3FGL J1518.0-2732TXS 1515-273?ï÷#DþŒ¸?DŸWméÚ?+RO[Æï?›Þb=?LžW:dþ?B!RdÝ?ïäJeåô!?j¤ŸB	>µ?@szU9Æ(?Mt|à?g˜»p¬þ?eVðåj?ï§Ë°x?aéÊù~Ø?Zeã]¬´L?fÙ9©,QG?'íÒ®F¥…?€-I)Êî?ïÚ)G³.&?R+Âß4ij?K²Ã£%?0yª"Ê'D?ocù6?P)]$ZÉs?ïò-î¿¡?PKt97* ?6ÊCG+£?,ç_K3°L?Uñ'À@Ô/?KڏAc'~?ï´ÚV†s?'ÍKt]û?OœÎ?_†~áfÊ«?€Ø‹/1;?Ò­0U*z?ï'ó=,ŽÝ?ƒ˜øAj7'?^tð§¦WW?^V¦@?‹t'¬žÍ?'¶'µÇ?ï¬6v«û=?mÓ¶ôê<?_êŒ$·×Š?K<´n~N?€õÜá£?j[¶*èAGN4FGL J1518.4+0750¿Â}OƒmTº@Iãø¶À;¥Š6OGfÀ<϶4ÚÓ @!æ©ÎÅöD?øFc[ïêß?ჲ<'Î{?Ñ[Þ£ˆ?ø@¢òÞ¯M?ÿ8n±d¿ï«¨Å†‡n?Öo'nÚ©.?ïኔC"¿À"¢Êšî¿Æ%
€œ¬¿é5<ø®ÒçAGNbcuNVSS J151826+075219?ïŸCñ¶*
? qHó[þ?Y&HÙ،ë?P§e0¤t?…
:uړ-?€—{Áî?ïÀ¡Ê"aé?}b7؉n~?PBÂ
n{?Ye?i‰Eã?{§ÊÇ5?xü@;»?î§~"é?"`>Œ¶9ì?r´¿Õ5ƒ?xŸ_Ckìa?£1†¼›qù?"›ˆAö?îìhTìÛ$?'Uÿ|"?WK¬Ymb7?G2×¢é? MŠû±?'–Bž¡?ï<t''&G?^'¼È¡.?jêo¹$ý?bØAýÕÉ?•Øɖs?Ž#ƒ5ð6?ï8Z3ŸŒ?˜­ú™úV?cʬˆHT?pî›QFC?–{cö

?–œ7p¿Â?íÞfP¨U?…'ÛÒQ±?rîd.û+Š?sK_Vs?¯»ÎkÁË?œÞjÇj|?í":9Œ¾•?žU_<'e–?VFyçm§?\p'?³LIKý?ž€¨ûÅAGN4FGL J1518.6+0614¿ê¥áÚ:@H¥Ç%ÃÞèÀ;NÉ&O"À<¤À²W&@!¶¿•×˜?û·Š*ÍB?È8uý³¦?")ê4;ÆÖ?ÑÁ߇Oj?ýÓ*U"¿ïðrXâð%?ïÿýfG³¿ä·K%˜?ý¿È¾ð€±a¿â›ëþì.½¿¶W¦Úõ¯oAGNrdgTXS 1516+064?ïÙöÐù¤"?qB›­.oª?8hI?"?0-£ü}?q~ÜNëŽ?qöù"Á?ï¹ñž›êŠ?}'ªˆ}	?RZ÷+ŸÝØ?ZœzˆÕüŸ?~pråÿb?ye—û‡ð?ïeùu'€?ÑN'ßz?a!W¥a÷?]陛ûÔ6?'¦m¬D±?×T¢['?î¦Z3lö?€À³+>†É?zÖª‡*¾´?aûþ9"‹ï?¢?‡z>QÎ?€3âÄ$™}?ïÁµäAÍD?n7«'Î%?Eªs¢ÈÖ¨?9<8°.­?|o¿]|ø™?mh.É÷?ï)Ã|&?•'ä»ÚJà?d©©ñ$?jLLAö'=?˜[bg°?"lÿW?îô£QÃ?‰aÑáq	?fÞMi­?]Âl¥[v?žÕ–7?ˆwƒØØI?ì4ŒävÙó?š7UYÜ?ʦå"?}½-sÓ ?ºVæ3Ù©Þ?™<ZèóÆAGN4FGL J1518.6+4044¿æ[k½#@Lp'À‡D,À:¢"O…yQÀ<¡ã¼Ó[@ *4~6çž?üÕnvÖ 3?½ãpþöÌ?¶Fçeç¢?ú£é~´;@èîݘÌë¿ïýI׺f™?ïúþ§°´¿ÆS&ƒ!ˆ¿ÜèV*¯3¿ßìÑ$o¿Ù<ƒÿS‡¼AGNbllGB6 J1518+4045?ïæ^x}·ˆ?W&ÞqÏ?D»3ð,?1—¶Ûa?dŸØþTsf?TÎ;ŽØ¿¯?ï¹ðHŸM…?%ÝPÒÒ2?[ÂæŠ/8¾?dîöø*WÇ?|"î7R?wN·G{Pñ?²Ô?tiô|Êo?a"hx›'?`
®ü¢"k?ˆ›?ù'½?r½4Ѐ"?îöµE
ë?s<-j_Üí?…/d½1ç?gSÿcÔb?–'¥<è¯?m›‰A]qŽ?ïÑÓÑgªù?eB'o}.´?X—Ø" Fé?NvÝï
?pð!=ÏÝ»?bkN-`ê?ï6¢ä'n?"Îr"š?n`x/Ð?sçäK®?•kk]Ð?åNaÖÂ?ï7Ö–mÚ?jd~ü?k:ٛy?fE[LEL?•¤•m‡dZ?~¹Á·'Ô)?íô#A½S?ovsF?•Â¬YÝ
"?€D§q—÷?«?g ­r?ˆ?[¿×AGN4FGL J1520.0-0905?Û¬N֘ö@CwÏÃøõÀ:ÌØU—À<W÷øʁ™@ Ú³€ ?ÿ'º¤ê?ÇX›w•7à?Šû«Uè?Å™bg(@«"ÚJŽÄ¿ïÐ/",z²?>·Ë´¿åÄCá× 
¿ØóY^@'7¿é§Û?×$¿'aAGNbcu1RXS J151959.7-090434?ïcÄ~'V?® ÅNQ'?i¼*³®?}¡E†?™|+"³u?ª"¨â0
?ïÁ)S5‡?v±
=}â?Rbžñ S?Z{Õ°4?z•'̃?qø0ÊÃs5?ïGèk± k?…³Eä§@?mƒ´ï¥-»?p"‹ËkFø?"R{ñêÖ?';Ì-ncè?îÊí;N­?}±8ÄÝ4?€Ti@?di­›Á«?žbÒi6'ï?{½ù*¼Ø?í¯;Z&Ś?°çt'ñ§ò?yÄ‹]?kÅrUQÿô?°éãÎ"
¸?°¿"S¦	-?ï>X?"žqCøÂ?gîÿג•?qޛ¼žM?•2=ñ¦k§?'ž^'l´?îsⓑ€?"ìÃlŽº?w½ðà®#:?tv'ˆô^?¥Ê­ïé'?'›ø³I\Ú?ìÊ.÷±ŸA?•á/X¨Ð©?"‰*­õés?'/Œ×YD?´Ì=—c?"~p¦ä¹[AGN4FGL J1520.4+5546¿åäÎd¯g@Ilë¯#À:‹F¦­~SÀ<ÇúȈšn@29¹µú@'DEª.<?ºªlЍ̇?¥1B#Ÿ?çͬ[==x@²çôE¿ç£¥€š¿Ü	»€Hj¿ä­ÂC±Ü¿àAöD•[F¿æ ß=Ù¿é§E‰w§AGNbll3FGL J1521.1+5543SDSS J152034.98+554256.9?ïÞFd?e|%îÃÑ?QK"IÔ?GÆXÊ1¥?iV÷uÿHé?cƔ¯ç?ïÍE~‰•?u½¤–šÝ!?LêPY…þ$?U":°60?uÀ+ÁZÃ?q××ÿ—?̈́r?rRýùùU?a³À '[á?`hÑ0yçm?‡íoðØä–?lÈ{´uJ×?ï­0Ÿ5?_éØÞt?p§Ã¾ß5ô?OÑ='Õ{ý?x¿õ×½«š?XT$þ½º?ï¼?8¥
?u0ňsv+?cDäKô"?]3­x"û?x=ñð]?pº"~h`ö?ïV\ßî¬_?"§ÿ꯬n?`JÔ©¹ò?gQÅ&³›•?"+M@—Î?'"ºeYj?ï"œ'À'?'>i€?p¸/Ž½bl?l´`_½?—~r½/øv?|ºo¨[Šµ?ï¾Zï?}ótWpúF?‡Ýc"-4=?o7öG4¾ï?'–£‹"?v"à:qyÃAGN4FGL J1520.5+4209?ïÿýÝQÞ@L÷< À:——sN¬5À<•B›†ä@]"s퍍@*½Bì?ÄûÆnäº?ÄúÒB¬?ùé˜dæ3¦@³ÖwñS?¿·ø·otØ¿è•*™1¿äö3kgW¿éÞá¢Fç¿è_Jþ«í¿ðAGNfsrq3FGL J1520.3+4209B3 1518+423?ïñPâñ|Z?WÛxO\µ"?@çÕ¶©`¶?A‹ã¼L»n?TêO'å¶?S©+á«d?ïá±î¥Ã?l"^úgáÐ?9—ÐCg!A?F_›&&?kŽ·b?hèkÄE8?ïa'XÃ±?Š³Ý`Åqø?ww1֌ø?ƒe¶û+?‹ãÐéIצ?"¨ËMàj?ïêídqð?DLɕLÖª?I¡g•œ÷K?,CÔ¯Æó?_q%ï?I?BkG$.ß[?ïÝ.Ž¨$?h"gU"$?Sª¤X?R†ÆOsõ?hüæÏ?e7Ë7ê?ULJ¾?‡
LLCVj?PúkÉ®0"?[|#1Ëc?‡zÝ1¼`?…OË Mž?ï#ŸôÉã[?†Ú¬Ï??x"
øAEÌ?A;µì?•g>«öä/?‡{G~V¸˜?ïÀm|‹?cÅ×óÃòä?`îhd€¥²?I¾&9"£"?w•
5‡z?bM=ÍjðAGN4FGL J1520.8-0348?ïýq—
âÌ@E@j]këáÀ9e¾¶‰"iÀ;ÇҝÇ%Ä@ ®ÏÑ?øÁi÷ë^ˆ?·5ëŸJÞ?Ȑ°|_!#@U¨¸ñ@zkði	.?ïéÐÒj›¿Ò±Ä}óË¿¿ÒƒÒ‡÷°¦¿Å"¨™Þ¿ßÞ¼¹YR'¿äܝàP7PAGNbll3FGL J1520.8-0348NVSS J152048-034850?ìl¤Å‹~¾?´®YtY{ï?±Ó¯‰Âw?¨7‡4J?¥¢F|Á;?°yÁȸ-?ê½ÂÃ+Þ?ÄÙÔÊ>Ÿo?ºæÒ¡;é)?Áž³ÅûÞn?®V.‡hCÕ?¦kœ3¼já?èÆ2>õì?®Ï'ŽˆO?¼~Ϭ§O?¥µËµgÙÃ?½OžùªÑO?¨6X@XÁª?äÍ7b?§Ù­6ؤß?·UgŽ?"R]¥4æ?Н
TÚÖX?§2ÿ©ëa½?ê î3h¦÷?¸	ûk$'?¼"ZüX‰?³؊+x»?¬ÖØ"v?§O(#ŽF?äOZӂ•é?Ð=°xûŒ?ÎÏñYôèö?Íшftê?¿åF°~Ê?¸E'>ÄE?ç}ü2ý£?±¼Ë\Ÿh?ÁæíàBË?©7ûY}å?Àù(F+nª?ªeÄgéíF?Û° uš¥¢?²[…ÉVk_?Á¤àÓ¦?©{GW¯Í?Ûō¬Ê?µõúˆ¨ÍÂMIXED4FGL J1521.1+0421?å­8TQ³H@GÖbýüÁÀ;<-šlþÀ<'ÐÛOF@¼ú%6ñ?þÝR¦–_?Ó+-€@Ø?Óµàaª@¡B‡N@:à\̉±?ç(-í¤?ïÿáÍì¿ÚÞ;õy"A¿âÄ»á˜
ù¿à¦ºŒ¥¿ïÿ€éŸkkAGNrdgPKS B1518+045?ïƘZ*Ä?•[3ÖÿÓ?`þòOòh^?qò·q‹¨~?t4>©''ì?'‹Ä#Bë±?ïÃÓ'ê±?väסbHô?R¯8ÒXõ?Yr$ÿžÉ?yjP¡È-&?r;z^.v?ïA¦d>(?Œz´¿jM?r˜bj3÷"?v*«¬·?"%àŽÈ?‰ ùð}s?ïþ\3T
?wõ\íҐ
?~¬²Äò?dڑP"?–3ÕH"?tb€K"{ì?ï·ÞZ¶&e?uvzý—…ñ?oEºj»²ä?jñuŠò?tmõ{íŒ5?jBŽ bOÇ?ï3ç]Pœ?•)è³gˆì?n~ÈùQ¼À?uÿ'†tz.?•³FÎL|ü?'Úâ°?îé1
Ó²^?'ï§Jåµ?w6
…?}+ö±(RÄ?][zÐ?·$Vçç\?í¥¥aà?"·ù+$›ì?‹ü |E?%wáË{?®¦¡¼i,ˆ?'XÞ¦Y"žAGN4FGL J1521.8+4338¿è)Ž¡Ãߓ@KÊÒ¡øã¬À:HÚgÀºÀ<P·»*ä@'fuªÑû@DEÅ.î?ÀÐd[õP?³FþÌX´?îÑÕJIÐ@#ö½8ÿ¤1óÿ&øN¿æÌuúX S¿ëÎÊϜ‹¿é^ÑF¯ú¿ïþÔ¡­dR¿ïÿøãúAGNfsrq3FGL J1521.8+4340B3 1520+437?ïä&Kª^Ÿ? 0uÞfmÁ?h_¾É­GF?Ÿ(n¼©Ç˜?;ϪIC÷?TíI͇?ï¾9¹¯Ë?€˜©H%?Y–?»åps?f½ž(n?z}°2Îæƒ?v³˜!å"?ﱂ¼æÙF?uE¹K$f?fÞ«¦ÊJ?qƒÂT¿C#?|52,q#ä?g9ã}ª?ﲞ'ƒõ»?a!Ó 4Ã?r-Eý R?WC>ŸG5x?tƒx»•§N?U—µ XD?ï»y?^·wb?]ýÕèA?]6°Ü¥^©?6/+Pí^j?6Lá :'ä?ï8ÐM'6?›§Ǹ?p-'­Òae?€Ùò'Çx®?˜­œ
šÐÚ?•Èéÿ'»½?ïyhEÛù³?S¹ÐŤ•?mËnö|Lm?rä‹Ã2¾E?Š3ǚî4?v8ԖE€V?îé¨ÜhÝJ?†µuz	?'èRqH×?#j}ù0?â'Uqâ?x‡aAGN4FGL J1522.1+3144?ïÙ0B	‡5@L'€uMÀ6¯ÐÈÚÐÀ;,âó¾ý@þH¸Uœj@õ¯¯…")?"}k,fˆ?²LDÀé§@&k9:´0õ@ ^œAk°¿Ð9wн¿â®L·2¿æŒï'zß¿æ»Ráú0ˆ¿éK·ž'QÒ¿ì]Ñó¹AGNfsrq3FGL J1522.1+3144B2 1520+31?ï¶ËӘ?z2‰ìZ¸/?a÷Qܜȫ?_'=²Àž?{žÔ/"_p?un®‡[	V?ï.Ä&h¨?›ÊÚ²¨.>?y5܍	•a?ŠÕô¶K?"ÚáV?•°§cló?ï`3bi<ì?'ç gÝíƒ?'Ö'¨h?ˆô[I6[°?…–Y`S?‹#ú«ä<.?ï×þ`ºø0?f5û¥€j?fe™riî?`@*?T5Û?aœ‰Ž¸­Å?SSqÖTà€?y_à?žõͱ€?eÉì2e'?j+†<ÙÈÞ?‰	h}z¦¦?ë‹\s?íôi–Ç'5?³Å\ã)P?ÁѶ8?¤Púk?¨XÝ)ÐÙ®?­å²ÞÐ_?ïUt/õ¡?'D-+íÊ?'`õ~æ?‡1e.¬1?ˆ""' Ú?‹{uÎ*ž?ï'ESã?f3N­«S?}b¸C?P;?v¬³ì©?yúÅŽÖŸ?r£Ë¤"AGN4FGL J1522.6-2730?îœ_΋'™@8fnü7£À8¯®çúÀ;"Ú")=@G'%\@·g2Ë?¦aPÒÖQ0?ÀBLUÄÍ@Ó:aû›@}*x#¨?ïJ?SÒåì¿Ý=E@¿áÆipÜáî¿âeÁ$øÞ¿égM·B÷Ì¿èŠS«x¿.AGNbll3FGL J1522.6-2730PKS 1519-273?ïΙ!Æò?kÌ\)§)?`9ý|2?V~©;b)?pÚ´¦C/?e3/R4–?ï°ºŽu"?€	<š01'?`ÂJ³ï?fÌ{-DÊ?œý·³X…?y`k
G$?ï÷×	4?–Y"¹
'ß?¯<Õ.¬L?ˆp¾…?ŽRÍon~·?Œ `pùª`?ï5>¬§Ø?t	•Õ:Á´?|5;SƯ/?`"ƒ;Y?'Q©X
/?nÑjÞs§è?ï¯Ü4&€Ñ?t`ӊm5?gÜ`î"å?c¸ˆUý/?|#µ{R:?nAR—'Ö{?ïè×Ö|_?—ÎtŠù3?z|e9%'?ˆÖ¾rÒ?•Ã˨QƱ?'Ò'­˜ßG?îÆ "´?›`f'É*?'…BüRA.?"¾ Æûм?"¦¬rQeª?'AúÈ?îÅ7›ç?ø·4ªÄŸ?'m£-6¤?y$½AD?¦÷¢)[4?‰¤¤U-…ªAGN4FGL J1523.2-3941?幞aªiö@,Ï9ó@ÔÜÀ:š
s÷H¡À<&« ,ZÒ@/b™'Y@¥D]'""?҇BlA?یo¤þ|@‡XÅÉ£@ÃNú#"?åg' Ö9]¿×9PC9e§¿á¸n¦¦ÈV¿é*è¬&d¿ïD‹ûbâ?ê,Î?=­‹AGNbcuPMN J1523-3936?ím³)ìE?¯›øL¤Á?Ÿ´î"ʹ?©œÈ£øa3?©JV<FR?Ÿ½É…·½Ü?íyWþ!a,?²n²æÓ?œÖÔ²·? œA&¬`G?©ÿ}·€Û?ª€oC]6?í¦)}…o? Á®
¿Ì‰?¡ÏîþÛ%?" ]×A\ü?­f˜y(Íä?–úèÊ÷c
?ípf¢Sä?Šb–!.?šRÀ;m4?v•µ=î´?«ÐŽøPÀ)?…dÌؽ?èãˆÏ®?¿q±™Ñ³ø?³Ó ¡¾´º?µEŒéªJŽ?Š)ŠÏ©?¶ü	ÆëEæ?éW2sQ(?Ã%)¦±t?´²Á$¹M?¶-å5aQM?ÀI×Vé?ºú¶TP?é"¯=«îA?°Ô#ýÞ{?³}<¨›œ?¡oj)Á#ß?Á¶¤È²òí?¨÷ai.?è	šõí¶?£u,͟x?±—Ú¹GÕo?•"g­'?Ç
Ð7»X0?¢"`
ÙW2AGN4FGL J1523.2+0533¿íEU©Íà@GùÆøÀ;$1âÑÀ<Ô{¦j@ BE‡H´@3c¿Âù?ÅZÒ ãe?q4a†'»‡?¬·øX$Ú@ƒ&ûíKÈ?ﱋÈö~w¿çâ³¾ÞοäӅþÝD¿Ù­_H•p¿èQrÿ&`?ÁûÃ	€AGNbllNVSS J152312+053357?ï¾ý"žeº?ý¬ìB@?Q›ùd==ä?V94‹Ä5?|7<ðßÆ?€àA‰cFÆ?ï†
QLN?ˆj‰*+e?c'~û"Úi?e9b¼S©?‰–\æDs÷?…%Y<™‹?ïc•ÇZ¥œ?€}ðl¡U[?d«E©8?nې´î‰¶?÷å¥í†?}3òŸ¾ýy?ïEc>"º?s—Y|‹ÕU?i(·î&?KóeË«™ª?"8PûÜ_?s{šp¨5s?ïyç©S~?Šð¡ég?a€?vԚç?^èß¼æh;?&ëTáÔ?ˆ¬ñ5?îåՀ`É«?œlÇ°V•%?h¯mÿ'?p"] -NB? ±=´?šðÎú?îßPÛÃ=`?‹©X~qJ?n%â췌h?pA>œÇn8? ("úw¾?‰üÃيՙ?íuã	WË!?"0%m¿úk?ƒŠEœ¡ö²?nCé|ñnH?±ßŸAb?'܏d@Ú+AGN4FGL J1524.8-5904?Ý1Pá`¿ýªôj ‡ÊÀ90êþ;·À;û¼¤`@ü†x)²V@¿:I§ê?ÀM^7?³Ï1VT'?òá+^R›®@=ÂKIU?ïqéQgÑ ¿äÜ-'€wŠ¿å'/ò?M¿à@RÖfª¿äÇnôªah¿íV ö…-AGNbcu3FGL J1525.2-5905PMN J1524-5903?ë¯7ˆ'p?µ‰æ¶<n?h(>ÔüB?b"Bãá?Àâ€â­Mš?´ÂW–ft®?äæá ‹]?Æ3\"ë'?sž+8
Þ?wSÕ\ÚY?ÕæbàŽº?ÆDø­{MÔ?ëF÷‹<_?®éI6'?Šk¶/ÈÏ?ˆ\î@Û}?ÂT(½À?­DSJ"i?èÞñýUM1?œYˆii?ŠÔ.i?¡»?e²V	
#6?ÊÖõ"_#?›'n•ðþÁ?èby.Àì?¼³ Q?ux>ßE–©?j³¥*9Ä?ÍÊYN"§[?¼m‰Êˆh´?Ü*Ór?Æ+ãH9Tµ?vqó[ۊ?}õ¡‹5<Ë?áƲÁlò?Æ
qˆƒqº?åbäÇüi¯?µäúYŒ‰?—¼ÿe«tp?‹}šÃ6âD?Ó¾fyþëû?´Ý=t‰ý‹?áO3¼<~-?ª	yüE`?~f›)M?~½+V#%?ۉ²(g±?©—'˜X"—MIXED4FGL J1526.1-0831¿ï·ôãí$Ü@C$Å~#òNÀ:d'>2j¶À<UW1?=-@ ÞÙꗎ?üèÀ˜áãµ?ÄÔ~\|W¿?ÈaZ8Ô%@2_¦XĽ@(jž"dÿ¿ïí¿‹›ª?ïøÒ¿€#¿ÙHÝòd¿Ø¸ƒ¿'¨¿ê Æê4¼ ¿Ã%I:±ÃAGNbll3FGL J1525.8-0834GALEXASC J152603.17-083146.0?v'y—?})\Ñ?n>•£&"?g˜k ÿÀÈ?'}ƒe?uÖ©	n&Æ?ï¶vÁtÌR?~‡ô¨Î]Î?`y"•Ï°?f}2'"ñ{?|·b|~Û?u@œûh–?ï=! êŽÝ?ŒØFsCþä?x«Š?ȟ?€Š^̔È?'0ù_6x5?†ý|ã˜z½?î†?"•y?{¸9áƒD?‰&¤>6?glÀ"ê?¡UÒôåó?vü¢}­æ?ï©­…V8?ÖõxG?‡\È ùFi?'*…e¶7g?'fE·ÍÀ?‡ð½œ?ï:B}öGg?–âWÐ*ã?pm:ÞÕ»A?x¼;ØçÃä?"œa'Îg\?'ãêíìyˆ?îuîækô	?˜ˆ‡¨ŸS¿?ŽJÐQÊI¦?Ž¦'·à—?¡]†…û?Þ®£K\?섒½B§V?"²s#EüÐ?™£¿>	t?} Í{Ÿ?µr¦æ÷)ô?'´D•Ó‰AGN4FGL J1526.7-1529¿íÂ)Þ!ß@@J#9ÀìÀ:¬ðéÇ´À<f]ú‡;@ |o»Ï¤n?þaÝ4ùÜÐ?ÆV©Zý?¼Ùz°m?öŠ"é9?ýÿrêg¹¿í$

[³?ï鯁7x¿ÐÀ¸âŠ#Z¿á},±8ò¿à	gB…œ¿âçsâOëÑAGNbcu2MASX J15264667-1530269?ï©Ú£
lÒ?ˆ®]Ÿ8,&?L `ij†j?O1›R't™?ƒÇQ&PH?†çÁ
š?±%7®?ƒ¾ÖøœIÒ?k.>±0"?p'©rŸ™?‡RCùçӇ?{Ö^÷ªA˜?ïrœå÷9?x'DªQ<?b=D¶•·8?J
‡Ólì.?ŽÉu'Í ?vè¡ßJ?íA^'}7Ü?ˆ­ƒ‰Ìm?'¯QY}Ò?rÅ|Ùgã[?±I7õú±?†¹
ÎB?ïS…°zþñ?™ZV·Ïf?_Z™ƒÈ?^­V'½}á?"™§ù‡)¥?—žR¯,?îÃÄ÷ãH?œº TŸš?|PhÏ‹?'Ed®Ã[ç? C!Œ?—ž*‡nòó?îòjö:{É?ˆð˜}¬3?m.sØUFL?^ÈoÛÞI?žÒé/?†½^1óôØ?饺»8‹ô?žu·Hú?¢›v«Ò?‰6¡6Lì?ÄæîOî¼?ž6€ÌluaAGN4FGL J1527.3+3117?æt¿K¸@Kò`ÐÕÀ: w!ŸŒùÀ;ù"GÁ`@Á¾V<"@;`äFf?Æ? fÒÇ俯ÈԀÜo"?à¡…÷%@÷§f‹Ð-?î†'_8u¿ëIé7'¾¿à§û\,Q¿ì#ã@Òٿłìƒ÷Eò¿ïÿ÷fÔJpAGNfsrqB2 1525+31?ïÒôu¢k?t—q7±
d?J¨â!åÎ?J_g/Y»H?s0¨Ôöî?rì9»Ö4?荒³S݀?˜Âe¡·¤?UòP]ü?a=yLûï?'"É0L,`?—ޕu"?î±JhŒŽø?•vù]Xބ?q.Wݳ¹#?vøÙ_ +1?¢ÅŽzb¹â?";KÒÞ¬?ýن?o"Å|óÜá?I‹ <ì¼S?9ß'¦°•?‹=F©Ôòƒ?nǑÓ=[?ï™á)"c?‡YùoÑ?`~'Ùºú?aGT •V?…h¼1³?…Ý/dX?ï?3»)n?ÖÅÐØjÓ?Zòm_oÍP?iOÁñ‹ò?–jaÅ-K\?œuGpP ß?í‡É**öÏ? ;ªä»C?†gòš¡2?†@¬üȟ?°ÿÉ°Tõd?žh!É˲é?îZëûU@?'"¯¸Ð}?g&u!£t?`í:Åìd?¨ÞØü¦œF?ÀHDæAGN4FGL J1528.2-2905?î8שcñ@6d)¿*åÀ;(9Úí!À<Rӓk@ aOƒöÅ@ž¡%Š?Ç{¹ßµ1Ñ?"'Ë´êz?ÀBE_Z®w@kÈíºX?ïo×ÿ/öh¿ç¥8ž¬þÑ¿Ô܋ò)ô¿ç…L»Q¿Ï¿'ýs2Ó¿çV¯¤ÙšAGNbcu3FGL J1528.1-2904PMN J1528-2858?ï3[=Š?Ùà¿DV?Z6qëý'?Q¿\*/î?—òèÓ.3ò?vËúš…?ïU÷òW?'6'mäý?nŽßÿtë?rA3j}YÂ?'Š¤øâR?"6?îò˜"öúô?ŸÂ«ö8b?k5y)Ó?iŠ@j¨\?žFL€ç:?ŒG|GL?îY˜*a[?pðäŸH{?eÊZÒƒÀ?P:A‡étð?¤ÍÀÍ?Y薼Kt?íÒ;Ր¸?¨â¥8I¢ª?k'˜lÀ??_J&éõ?°"êh9Ä?¨ ¨«« ?îo,"ø8û?¦Ô|eù{y?uîß«¨Ž?"GBË]â5?¦OZ·)Ï?¥*óm§Kª?í‹K‰Úùz? ~әÀg?v	ìBÖå»?mqÏw½?²Eë"ðV?Ÿß†VÔt¢?맡Aƒ­õ? øh@8?{³fûèR?p+û^#X?ÀƒßŒ›É? ëù¨ký&AGN4FGL J1528.5-2240?± ¥à |ý@;bÏÃøÀ;7šr­™À<¨©Û0=@ÄøqÁ8o?þ#¨FÇ?Ԁ#[¤Ák?äê<ŸB¥í@SÒz‹·Y?ùQµ)mÇ¿ïÿû˜'2?ïÿjÕþпÂÒ練'8¿êRz᝔P¿ç"Ü0¿ïÿ(3û°AGNbcu3FGL J1528.7-2247NVSS J152834-223522?îôŽ¦æ""?¬åóü?ztÛÒTÈC?‰
R¯É]Œ?šÐô."˜ª?ª…¾Wrñ?êÚGÓÂùÿ?ÁPìÓ8²à?¹ßlÁÕ"?»ÃWÄÑÅ?®œª¦IdÕ?£ò	ñf!W?ëæT½òii?§›Dþ,ƒP?¢ðA¨áô?•Vó$ý?·U9ONi<?¤‹.Î
ó?é	½²ž½?¡%4?»H°Õ?šûDéÅÕ?¼jÂkC?•t7ÕòJ?î¾TÓ°°?¯%Àþ'Œ?‡iªäP¿9?†Æ'³(U?¨é¯ù°Å*?®ihE´?äô ÃÞ«?Ê5ŽŽR?Ê["IšÂ}?Æ:d'¯?ÁÔ¥3UÂÕ?º»~þ…#?ê‹ç:q?¯öYÏYc?«Œ0¶'^ù?œµEý»,?ÁÄ5pò~?¬ Ì5D§Ç?ä-°løY?®uy.?Â,>³¹½?ª[¹YëhJ?ÍÃ6˜dÞ?¨d}'ƒÎøAGN4FGL J1529.2+3812?Ù¾¢p5{@K¤÷<ÉÀ;ŽõѨÕÀ<Ò¨Rcz@^{/v:D?ÿ͕I¨À?Ég=üºÑ"?ÁEûø3'ä?ø"¸vÔr³@Ë܌ÞJ¿ïÿæ¦Sf?ïýWÿ›V2¿æ3߀ƒž¿Ú
˜à66¿ÝÒ	L¯Ûû¿ïÿûbâMhAGNbllNVSS J152913+381217?ïßdç¶2,?[51Ëäj?Ny–·"[?CåÃÂCö_?hü²ºE?^?U™å¨"˜?ïÎYÝÊ~œ?u5ø‹¾†?Q*x£d§?Y™ÇÅ9¥?tˆŽBÇ$•?p»yw¸?ïQ?áä®?†L¯·çX+?cíZâ}ÑÑ?f›Åšˆ¿È?"aL©¯n÷?…‡|Õvf$?ïd¯²?i5^
ì$þ?}õÁ¢Ôl?`>…\¯Þ?‡Ù;+¹X?d—‡\\w§?ïÃyðíú€?jóɦګ?`Â
ÁÖ?XtœÂÀoÌ?uâ9¦Ií?dÉd(Ƹ)?ïUè©»ê?'šOÇÊvµ?g©žùm¨D?qÔÀÂ""?'hocŸ´?b³&ÔS?îèdÉ5ò?RhՐò?l5–ýjsñ?j%S©±{?Ÿl³úœR?ŽVT5ça†?î|GZ߬?…"£+jq?¡e`š(?z•ùÖl‹?ŸÕ¯Z²9_?åYÃæ(AGN4FGL J1529.7+6733¿ï]>ù©¾o@E 'RTaÀ:ø+ìïÀ<Ú]^è@#f½ú!@ÕÓ;{×?Ä:Ôd¬R?³En߆¸Á?îï–ü0g§@•ÀR@Á¿ïâwú ø?ï5Y³Ð|…¿æíUj• ¿ãËЮٝ¿ßÞÖd¦à¿ïÿ€ß֕AGNbcu3FGL J1529.5+6733WN B1529+6741?ïÞŽáÁ?`}ñÁz"'?H2"vØ?9l|á.Ÿd?kìX®™è=?]È6Gâ-6?ïÛLoh\?p+wà[ÔÎ?B™çòEË¥?LÕ¢[̝?p‹r¬ö9?k9¢šÀ|Z?mó3Ð?y@8Ú³"?bM"€>?gyÑMs$?‡I¢íGš?vD}@D)*?ïÏ:xªÐ?U' HVÓC?a§2HÑyá?FGMp"4¢?o¯*?Qì§p5^ê?ï®XXlå?wñ
ûìw?Y-zàdè?Mbû[ÑfK?Uº˜~þÄ?u"+8IÖ?ï'5ܨ.?‹&zê·+k?Vë1E) Q?`͋HÓð?Œ•"›É:??‰†¤¢ËÂB?ï#zen;>?ˆVÖB56?pºdû
X?qÞöopf?—‰ÄºY­›?…ÓE÷Uîf?ïõ‹)a?q¸¬‹Ó‡?uûH|mÔ7?aæK1ÚS*?…:^[ç¸?l¥Ä
<7AGN4FGL J1530.5-3026?ï¹(Ž@†@5öè)I¥À:"¡°¿P
À<IŠÃ=@ Ûà­T@š¶ÐF?Æì,c‹?º?Á¶Ašÿö?ý,…]T@˜%Ùç½?îåA7Ø´b?áuD C¿ÞA&¦\ö{¿ÛìVÀVë¿äUÜär¿ïÿséèwAGNbcuNVSS J153041-302559?ïº0ìº?oTJ,»t1?UtúE†gþ?Id
JbÆ2?}ŠKE•4×?lQŸ­yš?ïº7O~?xv…f1?`»¬é(Š?oðåY+W?zàô½¨?uØfÒ?½+͗?wü1D•¹?a´&H£6Ã?dr2Œl!ù?Šñ&«^•?u6Õܘ?îeX¼Q ü?€þª^p <?Ž¡TV¢Ï?l|\Ù%•?¢)ó?}6~VDÌ?ïiíƆP€?ƒ0,þ›½ê?ky•àH?b?[Úü \?Ž¦Gk¾-ç?KÛ·ªˆv?ï"@®_¾?–ŒŽ¿$q?tñFñÚb?|0®iüpC?–{˜yIr.?'özïU%?îñ§D§ú°?‹{s.o?qñ
¨ j?rz…/?NÔ/‰ÞÐ?ˆ)S¨¢	Ð?ì$¢‹¨Å?˜Ò\Ý`? Ën‹ s?‡Ú!•á^?¶u4ZɦÝ?"ÏëUÈ
PAGN4FGL J1530.9+5736¿ìL©€0UÍ@HUŸ<pɗÀ:¸Òñ±‰À<̋Ջ¸0@$֐šíW@8‹aÈqô?½+¶g/º?ž.–¸¶ã?âTæA?ýS$Z'hÐ?ï bb ´¿ä	£ý˝M¿Þ†\㔏¿äí·(Ùº¿É$û(Õ·¿ä+4̐fëAGNbll3FGL J1531.0+5737WN B1529+5746?ï—TUݽ?zŒz´÷<?a'äÕëL?SFòÃW‰N?…Æqtÿ‰Í?x®m0òö‰?ï{( ·P?ˆúqÜÍ\%?f"k^¼?hίW_?‹¯öÀJº7?"؈ûcN‰?ï9þtBO¹?†ÒË۞?ið¤e«?kA•µ®(?•'äâú(?"">?`%?ïG°Þ"°(?rÎøáQ¸à?w$Ê@XW?_³'DdùŸ?'@±©Žaá?p©[î
E?ï‹
WZ?‹H&nÛ~6?wôùç5!?rÈÖç6">?–1`>;÷h?‡N?î΄üdÑ!?™¼×ŒCoÁ?sYÕpùª?ys±ÚKo? ¬u‰+þ°?—L²Öā×?îp¬°¢Ÿ¨?"&y(šYÜ?vFÐø—27?s£SUÍÇ?¦,Z̻٘?'®Æ`þÇ?íµ‹ß-?'6Ç̹ªÒ?Ë)\Ãñ?€3YDO[?¬I¯ò'†?wœf3AGN4FGL J1531.7+4710?à0w'(~F@JpÄÑ¢À;:›!YÀ<çK,N<¤@dªrÚ½ü@ƚƒ¤dÏ?Ä[}i¸*~¿—ïY¥ÉäÌ?ÔsæÂer?ó݋s¼e?ïf[~«Ø¿ìB¾$=w¿»òRÃFfA¿ãŽc¥ÁÆ	¿â?~e`¬é¿ÓS'úð̆AGNbll3FGL J1531.8+4704SDSS J153139.78+470705.9?ïÅ+‡‡?"Á'Ì
 '?eSf¥j¤	?j×ғ!¿?†yÛhdü?'»fžž©â?ï.iͬ¤?"ŒK¨J'?vðÜ`Î[?y7µ#¼á[?"q»Ç%tØ?RLÆ/¹Q?ïb1;??‰º‹öò¸?tê'Iºe?x>êaÆ	?—ùbƙŽ?†R¶÷œ…ç?îׇF8|&?~½FqG?†äh€å7?p­³19@»?™œâñžµ°?x‹¹ÖÏ#?ï*/	i‰?"iψ†$[?m bî-5ë?hÞÈî?—mߺ7?"½ØNqcV?íÝ·'–i[?°è/w
"ì?"ŸŽ3µ"?ˆ§›…š?­"e¤'Rl?¯ÅâuÀ?îB™p\'?–Íx'îý?€'6Dm?•7××Å?§Ì¢é *ó?"؁òðL?ì˜ Ä¨ˆ?›:ÿ‡—þ?œ«wuT?Œboæá®®?´:°!¾?—´ÀXΌæAGN4FGL J1532.0+3016¿éqŽ–Â_ó@Kh'£"¯À:ܵxqÀ<\…íë*†@ÐÒ=úâ_?þHH¦4?µ¦â­^Èb?šrFQэ?ä‹Lš† @	'öWµžˆ¿ã¬,ÿ<‹¢¿Õ¢Ô€ËA‡¿à=Œó˜ép¿×®Ué@ Ú¿ãyˆíyë~¿ÝÑLcZî8AGNbll3FGL J1532.0+3018RX J1531.9+3016?ïóf*<¥´?E9ÂUˆ?0C<[7'? Cº8v?U"Üó'TÍ?BŽÁM-!?ïØz|6Ì	?q(ö5ªE‰?F"Â{Oµ?P±øÏvÙ?pþ]Š5(?lÜV¶zºÙ?ïȇ+¿Í?aŸ†¨Y/±?O«{ÍÂO'?6K)~¬ÜC?wÆúˆ™W…?`iS*rc?﨑4¬k??`;Ê5hé?_!
ž¨'?=c_øã?øn£»Z?^W
m§Ôj?ïëPãi¾­?U^ä-èÏ?=¥ vüî&?.7  _?`úx¿tî–?R‡°$©
?ï‹)œ[•Ó?Ü4¹Ò?Tý&ûM-ý?`È(Wê?Š•ô(c?Ö8`—)?ï¢m3ØÎ?q{ó˜Ìì?X,IW÷?Ugf¸9 —?"_/ÑW½?nlôcÙ]?ï/ƒü#}?z~${eù?s²Ök¢Š?Y@&¾â$·?—íŽãøÄ?xD_]
*§AGN4FGL J1532.7-1319?¦ñàœ@@Û$Aþ¨À7éï®y$¯À;iTJ0@½†QŒ@‰~Ü~ñx?›D§¤Ê$Q?º(žYÇÇ@{•"d~@€6ŹÞ?Ú¡½àåοÜü""+É2¿âc[Ÿc6¿å
î \+z¿åTw·¿èÖÍÏ2ÙAGNbcu3FGL J1532.7-1319TXS 1530-131?ïÛTa×
"?wç£ù&?P¦Á©5?T°a´‰_¿?lX=ÔÚáÛ?sR-—S?ï¾ÏšÌ8l?€,WYR¶—?Só|úՆH?c({ÒÞ?{›SddT?|	Q¢Ì?ïlŠ7&û?ÚA¦ÿ¸Ñ?ƒÈý«D?‰•Þûõ?u#Ü
?'8¬^`:*?ïë7êZ¯×?K'R@cáÐ?>URó8
¤?.1[3Î?`ýkŠA~Ò?Gb¡y¦£Ý?ïÙ
ÿiz?hfÏ1á7?Pm›)2ɗ?NO‡G†/Î?n«$ký!§?d­OÇÿ	?ï[ŒÌ4T#?"¾?g{zånm=?zûúIÎ#f?'ž÷Rü?'Šcƒ£‡0?ïXÓª¦K?è‹Eù{?ƒÖt°?ˆ|s`'?…õҎg=?†¾jtÃu?ïϊÜ`<?e­]Ç·‰L?OVñ?AÌ!Î&T+?tFîUÐms?cÓOE'|AGN4FGL J1533.2+1855¿âY‰fE¯7@JóFí$À:Y-2h2À<Y´E‹@ ú$…ñF)?ý
fóT?¸CÀ°E¿–¹Æ_ËA²?à'ß@lך?ò,{Þó•ä?î_8	[ÉT¿ä3"âz´¿àù&ÝdtŸ¿Ý…¥;8eL¿Û¢†\ûـ?•_m"îžAGNbll3FGL J1533.2+1852RX J1533.1+1854?ïŸÍêüZ&?…þthm%?X|Ãÿ*Že?LÕ5ýÝf>?"üìÎjž¿?…¶£v¯bB?î´¶%@O?£Œ>›©æ¯?‰7R†ój??"
Ë.=àH?œÍ'"÷?›AvГl3?ï`¶Üv?‰(9Â?|ïóÃ[´Ý?~7îçÓ[+?•¸£
?"8`Ë+?ëNåì.?™S¼s@ó?¡/`¡È–?'Fæ·?¿Ú7ˆF?—	úˆ—?ïN~'D´Ý?‰ay"+ö?mIVøj£x?coîæ­<œ?'‡;Gºæ?‡6kÄ@®"?ìt¬w—¼?´úmà¿Y-? «GÝ]jt?¦	&AÎ¥—?´øV¹+M?¬–dû
o?îM–&P)l?"… ,I£Ò?†çA÷?ƒÁɐ6¬U?¥¡£ÍPà€?ÆôÜæid?ãS.)G?«Ï¨G§÷?´
—•Ýi?¿3éæÏ?ÓÞ³¾w¹9?­¸›ÏÝVAGN4FGL J1533.2+3416¿ÐI°fÿW@K\
è³³À:4nµÀ@ÍÀ<tݒîY@úŽñt÷Ï?üo[Ømë?¾Q™Ð¡?»Ê³íض?ÿwÑȵ@ǙÚ\,|?ïö&' ®·¿àׇB_ ¿Þåqúfä¿ÆcGãnyÛ¿æ+iÀú)¿Ù=Ÿ¤u–AGNbll3FGL J1533.5+3416RX J1533.3+3416?ïÒ-ŸJˆ?aʖ«Ä?ImR Ÿ#?8yÐåz)Ê?s·BŽ¨Ij?^æpª¿‰&?ï³ü 
]?}îD'·~?^m…W""?dE¹ð¥Ž?~â <V¸•?vÂÏàÒ?ï}ÑuÄ?tÇ»ÖÞ?a¶I1?VðâÚ?Œ®XñÈ?r8µ©©?îßÉÜ#ú?s¤Ð²Ê?†*?è¤ùÝ?cL#ÈÌl?˜úæØÀ	Á?nêKt§Í?ï¶#E)Ö?m[â=%‡?Vw‡Ë+?C$9^p»?NÄû)ÿ?ku5Nÿâ
?ï&J±1Ä?"ÞüáMÉs?ljdSbçÐ?rì'[
¶?—²ª°?'[!uï$?îñ'+2«?‡ÛB?ò\Ÿ?pÕo£ü?em¯­Å‡?ÍB9Tm?…Þ¦4ú·?í'a'äk?a19o?™Ó€±;®?@ﵪÓ?°Pad¹?ˆ-A£¹XAGN4FGL J1534.8+3716¿ï|Ç(žâ@K"^þ"vÀ:†®û*®)À<{¦_z¹Û@ -¤f&O @h	¹½%?Á…dXo,ß?tWíÞ²€Û?¨üð-¢P@®?aê«°¿ïþöë"Gù?ïû³ÀsQ¿çác'Å>¿ÚT°ÜVW¦¿ßaÿÏ¿Ü3oce*&AGNbll3FGL J1535.0+3721RGB J1534+372?ïézÕò?]kŸgç(?>°.Ř=?2kb»ru?cR"'?Y·,âï?ïܑ$nãý?p\M|ôi?CTå
«Ùÿ?MH7R—Ú?n™¢	Ë÷ã?kîë«kEw?ïŸ{U‹Í©?{p-s°mÈ?S5V:›×?Z2y²Cµ?…ºâ:.?zðU5ç—?﹯dÃ4Y?]YÛ2û?^Cé¤3?@Nɇl?{"üÀŽ²¬?\@&ö3Új?ïØÍÍŠa?ižaµÀ¬?KÍh;S
?Ab
}HÛ?pleY¥&?f®±˜»»"?ï•:"‹??ˆ³ŠzÒ?PÚ¶.w¥?Z{¥ Šì?ˆ–°?‡9ï>^1?ïS‰}Ja+?"¯gp®g'?Zh™E…¡?]‡j#֐?"èFÆ{'?ƒëW–ݯ ?ï>¹dâ$?yj;Úäùý?tZy¶3à?_³m
‹é?"=åÖÃx?xÀ¿…¶îAGN4FGL J1534.8+0131?ìq½~ór@Ev¼ÿ À9‰èK®TÀ<½ÅÈ̍@ÆÑÄÙ8k@-ú¡ò-¯?©ã,›Ð'º?¡‡ê<ÒG?ó-ø–2æ@:ñž"S"¿Ì¦bÀi'¿ä­ºþ™"¦¿æRÎÙíFÀ¿åù?¼ ¿æneÆ-¿àËVq_iAGNfsrq3FGL J1534.5+0128PKS 1532+01?ïõ¹sºÈú?EåÖ×ú‡?'ij.¹)?"½p¥?QŸëx¢"¿?DŒìheë ?ïáLÔ¢Œ»?k9\³>?<1
Šì=ù?EïH¾+?k-
L!¨/?hduÎÍÓ¿?ï¾KßÉÌ	?gˆ†%»QØ?TÛâ¯,;ê?T')ñg¢+?{£jx¥?e7VÌGQ?ïû°¸Íš?%7bdÒY?,¦
ٚô?Ó`  Ç?:ï9(†?!V)j{?ïëÕ]°F?Z/š]Ÿÿu?4Yíù
Å-?)ŠmFGi£?aŸ¨Á¨\?XW"¤´î?ï©EØ7 ?ƒ¯-öw†ð?Néy)·?\GjQGe?ƒËVè0‹Ò?Þ_?$?kCšß?{¶ë.wº´?a&[|Z
?c«-UÑ«?ŠLNQ
£a?xâ±_càÌ?ïõž3S·?DCΝ)Q0?4z/Ãè=?%JÐè/î?P¬Aô5J?A=dPOróAGN4FGL J1535.0+5320¿ë[W(ÆÙ@I;:h²À:ÙUvT4À<»×¿o8@ ¥D#ñL?ú¿Ãvâµ?Æ»ª¦ds?ºs欜֐?ôŽ¯«SÖA?ú3–b'$¿çª=UËä¿âvþèÓ¿¿ãOb2Ôi¿³à}:"¿ãc܉ٿÏ%ï¨ÄÚ»AGNbll3FGL J1534.4+53231ES 1533+535?ïÐÁï#8ê?{Iµ‰Tî?=:ÜØR?8¾<!Åñ?uËZ½Øì?yõÆxs$?ïv-Cã6?‹\Äò¥ÞÓ?g:oFš¨<?ioXš?Œ¦5Íþa?‡¶Ø³Ù9?ïlH¶…Á(?z§:ˆéPm?cQ²†AÑ?[Ã=6T@m?>þúc·?xM×½¬I?¢¯©?~/¼ »?K<{?dB[ÖW ?¡e3{éþ?{0ɾ¨ÜS?ï±½\
êF?sLŽ1ÄÔ?H—ÇYohm?@ÿ'e&"?',—ª*‡?rL ¹;Ôü?ƒ}ð¾?©0}ó·!‰?u…퍝q?z¼	í7{?£æ•è†t?¨é5tgA?îõÙèXm?ˆÓqên—d?pW¶îI¸?lµAÍ;2?.ÕU‡pø?…ùœŽ–†??ìF»ÈåÚ?˜¸<ᡉí?"bHùå?'6%ϝ	¯?¸·W9øŸ9?–ÿ>
½ù>AGN4FGL J1535.3-3135?ïý­¾¥ÓË@3z'Ä"BhÀ;IØ›ïµÀ<"ü4µê@!¸îžƒ¹?üÁÃiv¼?ÔKí~ÉÈ?ÈIW·Ìàn?÷:Y²ù¼ð@¤Ç¦È+R?ïʺŸ¹¿îegÞ`ú?Ö»&F»¦4¿ÉÌWÇg2>¿æåöŸ..¿"ì Çm3×AGNbcu2MASS J15352963-3133461?ï¢ç´bP`?—¾ŸÉš¤m?G"ãn2©·?K•6ñ?…ÌÔ¡°Óî?—•u·›¸?ï™ɀš£?ƒ¯×tIÁ©?_å0ºh·F?c{f)‰ú?…Ágzä~?€­Fˆƒ?îÀ!)_?–y]™K0¤?e!X‹nø?pŠvþôn%?¢uîe™?•¥HÒÁSS?ï7pé|1?su
?\ŒkíºÇ?D—îÉmH?—Iì).?róO"*O?ï|yùžÅ†?¥UPEŸö?QêÚD%¿?SÍøÁ©Jj?Ž¤&Kª^Ÿ?¥9œx¯Ý?ïÄA/?š$³âœÍ?nõn"eº(?}ŽÐy¿Þw?›ßÑ&ò´È?—²ÇûÈ1?íÄU½KÐc? •ð|0P?r¿¥#êÛ¡?}žCÛ³Ê?°±WÂDï¯?ŸÁfÂJË}?í¯¡€˜Á­?"Òå""ü?kÞÚcáÃS?a¦@dRÉ©?±£ý&B=?"·˜YVAGN4FGL J1535.4+3919?ì5¥NÂR@Jøââ¸Ç\À:ÎNCYòÀ<½'_Á0·@–À©ÓÎ@çÚaàŨ?Ã#¤õÃ;)?ÅÃ[Ÿc6@S,ÀRk@m‹¿ï‰«zl­¨?ïý_Üßiˆ¿ÝsÃüČ7¿æ¼þùoÿçdÂW(¿Ú¬‡]ðAGNbll3FGL J1535.7+3920RX J1535.4+3922?ï¬Pý+?'(ÔÄ;?fÕ47Z®N?g[oP¾‰?~m9Á?@bÞ«ù?ï¹RðÎðÐ?^Ñý¿°?^?-÷T?gJ¾÷kk½?{Ƨ±΄?uõٓ¶'?ïd¯cý¢Ð?~ëù‹cJN?n9쁑CÃ?nÖ¥[ù4?E«àâç?zC¹ÖŒ|m?ïiŽÌ-Œø?j+"Lîâ?"¼½{š+ð?dôæT†â¬?€ß‹8ƒÛ?]I¦|<è?ïxàTF±É?"¯4ÞY?wi˜‰G´?s
Ô,°Ì?†±?)k?€r\×E_?ï~­§e?–²Tøì°?s䜐´ó?|Ȟ9Èjì?—W+Šp§?'ÅÊ¶1?îÀ£èÁ¹¸?K+àI$Ž?	ßOëµ?}'0«¤?Ÿf"C$~ ?ŠEýŸ¯[˜?î•o~úD?…|"j'²?—L£FÁ…q?0"Rm´±?–lØCÄ?z<-ˆôAGN4FGL J1535.8-4730¿í¾iƒë÷#@Ô
ª}íÀ9òż7SSÀ;YË0ëZW@ÙQj€Ò@'þ?5Ÿõ?ʌ×ÿ°ÏÁ?ºŸlÂK¥?ñï_˜@Ê.¿çk(¢¶xÍ¿á­|5Om¿é
߆ã´p¿åd±û.·¿ïývƒ?Ñyé{VwAGNbcuPMN J1535-4730?Ç×? T¹W"à?Q"6V!?Et,V$9?¤á+1? +#¡ô¿?ëELß<ø?¾ÝÝÎRô?†ï¹hž[?ŒÌF#¬«»?Á{ÐñI®Ë?½鬊Ê?ì®UZqÝà?¢åáçôÃ?ˆG ÂF¥Æ?¯µL?·"apnH?¡ÏÏFäD?íŽêzBø?"Žˆ:îàÀ?s‹6´?WÁ0sÎ?µÒØfŸK~?"älNþWï?ë×5à¦bD?´«ûà¥a?nV½;?f¾­ñ†'Æ?À)ÎzÌÏÒ?³î["F™?æÌ`¸ÁA?ËÖ˜Ô?"nÔÉñP:?žÈ‰òÃ?Ñ0áñïh{?Ê:àóíšo?é(ßh
Ž?°:ÞȖ¿ò?›YmüÕ¤?'Wo$;xÆ?ÇñT¡B‡?®Ÿñ ¹êå?çW;Ñ€?°½{¤zÄ?–õùŒ‹y?xš
Ö½M?ÐdЮG•Z?¯=íEo<AGN4FGL J1536.8-3155?ïþm•&:@3…7âÅ]À:˜0òçÉÀ<MãÕ'b@éÿð:»@nÅý0B?Å ¦ÿÝo?»17°pu´?ù»aj~#@ý«Ï§º?æ§,ßÜôã?îŒðÿ1#¿ê¼'ÂåÃ>¿Ëùt`$-¿èû,=WN¿àm­'"ªAGNbllPKS 1533-317?ﶰ¨ÿ¾?y‡)¥Kñž?W)ʓ´j½?T™›.h?~Ý8é¢8Ù?v¬QÎÈH?ïËÖ³‰Œ?y1&ÇÄ?UÓºÉ]`?_K#Ø2ï´?tÏ1GH–?s("ûÊ2¶?ïIeùüRC?Š |vmüz?sÕLrQZ«?|PJB0ã‹?'Ýí¡ý—û?…rÇ?;¡Ž?ïT°~–ç?q'¸¶#?Ü?~»³å]Ä?aá;RI?‹v#ŽH¯Q?kmˆûÛèÒ?ïXBÕκI?')hP-?q²·!'Àm?t}݌žÆ?Š÷t©Ò?ŒÐC¡UÕ¾?ïfé`"ÌÖ?Cƒ×HMb?kŸ{'m³+?s('Ü8©?]É ù±?ŠÑ
î]?î§ëkôDá?–æ˜Oí~?€€hsót?'õÀ]"º?¡a/#fÞó?"@_6^pU?î+qÙó7+?Ž–.
/?–Dzz¼×?ƒR-/÷1?¢G@&þÊà?…jBi(äAGN4FGL J1537.7-7957¿àNu]>
qÀ3rŸb0wÀ9wJ‡ãŽ°À<þ–µº@Cƒbu–@Òâu«}È?±	]Ýçãe?›Z*‡¬Ëê?é´/JWè@'ntҺͿÆzðv g¿âCF;M³è¿å¦ÃMÈ	ï¿Þ5|c¨Ç¿ç»ÿTßUf¿Ùa¶ÔAGNbcu3FGL J1537.8-8000PMN J1537-7958?ïöaò?NÓƏ›n±?$ï՗m-ò?!Ìêo?Pž!X2M²?Jé"Õw½?ïçºGíˆ?oÙ;òQÈ?7èhDÐÜß?G†µcÕÙ?f8':2?l¨€.'ø`?￑ʕ?j¡Td`p¼?Q™ŠìÝú?9WÔ%í¥?{Ѿ¸"?ií6Ž$Ð?ï´1‹úZá?_®".Rt©?[Àþ²'ýñ?<CHB»?~öú7\U?\[î«?ïëÆ·X}?XLm9K?8ÊÃW+KÞ?-]Nð+y¬?að4TÌ-?UÝÒøŬþ?ïºÆë¿ß²?ƒ;=e2¬?JLÙÏd|$?_š5QÍq?RîÊ+'j?€Ø×KóŸÓ?¬P4?yŽ ÷Г?^"r³?S»'=ˆåU?ˆ›¢Q[äÄ?x‹µ®ÇÃ?ï5yˌʘ?V¢´¿o?tܺ‡!0?]LÓ†4#?"M`øÁ²?{.¤®¶7AGN4FGL J1537.9-1344?à˜"LÅi@@EæšÔ,=À;ý>" À<u¡gÄ4x@!ë¨îv?Í?ù6 hUSï?Ïô	Q¸Yx?ÌfÜX$­@WƐr©@ùìðٜi¿ïÿøsCÄ{?ï˜b'p?ïß°Ÿoœp¿¨îi t)¿äŽ¸Ê·H׿…ž:J…AGNbcu1RXS J153757.1-134334?ïÀçÅæBƒ?	Õ½F|þ?Låaºð?EHƞ§Ç?{ïp͇ܨ?€@97 ?ïÑ>Վùi?vŽ"Î ?OÎLTÈ~f?Y£†Hó?sf˹˜ç¿?qúŠuéT?îÿi"R¾Ð?'Æ®|_	?cŒ ¡–L?ef
§Î?¡Iˆ¬ƒÎ?'Pî®ôË?î¹p‰!s»?"þ#ýxJÆ?q–æ!	Íx?`B«n«ËË?¢6¬õ.$?ƒœb•¯%Þ?ÑçF~?ƒ"(±À{?V1Èe0Ô?KD2 ؇?†"'¼&K?'vŽhVý?ïm\Hª?"»tø´ãö?gš(Ýß6¹?†g^›-N?Ž²Ľéî?4 ¹¡{?î0nápY?›ºÊEýÈë?lT±ZÇöö?i"}DýŸ£?«3ÆҞG?›Uz n?íVëCQÛ·?œ6ž¤O½ô?}9©ÂÐ*k?w
jÅâ?³uJÚñ]?›´ÿ"JݾAGN4FGL J1539.6+2743?ï·Rñ$×@Jnž²gÇÀ9‡tw¡!MÀ<^c˜UÌ»@c"çQ@…¨¸ñ?®ŒÕ;d™?ŽÐ¸rwÂ?Û@ï~¨|‹@Œ+.,
O¿Ý UàÝ%
¿á±ˆmø+¿åc(>«	¿ã(c@Â	¿èQ¥^ɹó¿Úñ VL<ïAGNfsrq3FGL J1539.5+2746MG2 J153938+2744?ïø´x(kë?<\ï¦âÊ?!°‡up,?Þ+ù48?HÂ=¼‡?9Î	×æT?ïá<e-x¬?m~Îæý*†?=Ì$·Fg?Gc·ñ	~?kÁ…S¸û?j$—2‰?ïÀ͚+?hkQÿ
?RËËî¨?>‹ñâØÑÉ?zëF~ÏFÚ?g*Í+ìëÅ?ïüðˆ‹ Ò?>êð{?
:úZ?ãFk
Ž?1¸x1Üe?9A€NJX?ïòª&&&Ó?SA"†œõ?0"HU}P?$¹"L?V£/`½õa?Rutï;Ç·?ïœûj]ۗ?†ÁÜ#°H?OПû`Y?Y¬n»¦!?†ÄxV}æ?…4›Û@Ž?ï"EÅ.î?}¦eµ'Ý?aPñZXå—?bµí4±s?ŠšRsŒ¶ÿ?z"ôp.;?ïø^ÓlpŽ?=¤§Š?1•+bD?$0·=XTÏ?Eºäƒz•?7–
Y§fŽAGN4FGL J1539.7-1127¿ïˆ3´ØÔ@@ëˆe"¯OÀ:!4–àµÀ<"ý2Æ%ê@ çTWÆ™?ü¨Ö¸ÞÙ??¾KÞ'ñ?¯|©,?ñ¥×Ë-\@œ‡VKJ¿îê´^–ä3?×p6~—4º¿Ó3ƒ$¸:¿Üã'ìý¿Ýt ƒƒ,ƿفí`@1žAGNbll3FGL J1539.8-1128PMN J1539-1128?ïÇpU|ð?c¾
ë{?Q8#¦Ûóó?=µÜ…Û38?wùéézÆÝ?aã,îŸ'G?ï´;.ÜY?~¼¥½]Q?[XnÑ óÛ?dì
ÌEº1?U»Øº•?w
ŠD£†J?ïG)Áù?ƒ4.eƒ€?k¾
Íû ?d"~L4)´?"––ëûwk?'A6ç×Äê?í•Þ:LEî?ƒ
[XÑ]l?'™rǼs?bbÔëe"s?°ýßèìÈ?'MP–b±?ï}LP²íJ?'5kFþ ?f«æq
\S?Vh̉'Qâ?‹ò<€¶_?ª˜žŠ®?ï7ný­Q?'ÜGÍ¢t?géí ~#•?qg_ŸGºq?–þriÝr?Ýþôeð?îƒh9q³?"Uò!†g­?y¥½'—3?tO"Õý™?¤"Ä´Ú¥™?'¥¤Ɏ­?ê@IÑQ¹(?šz‡®Ö.Û?"ƒù'Ä?zµœÉ9Ó?Ďu=·?™õY9Ö[.AGN4FGL J1539.9+4220?á'×]Ÿ@JTøœ^oøÀ:ñ/!U»À<·Ö™Õ(¼@BÉ0`@ÞKÊÙ­†?Ín
å÷R?Ò¹·FRË@Ü$Ts@ž‰XöU?ïú	Iú¿àì5]YøD¿åÑ,½ùf¿ãVq_i¿ì˜FÉ))¿ïÿ韖]ÐAGNbll87GB 153741.6+422719?îß×ç5©?˜Kè~ªº?†\ÃÌßFk?Ω¼ž?˜Ö¡:au?'ºÃõOÝ?ï9žI©8?‹šÓµ²'?{_4FQŽ?v­0@ŒÒ?'ôi½Á"Ÿ?ƒ—qúÚÙU?î˜4ì4µÙ?"ï]J§Ñ½?ŒK@ÊÎÚ?‡ÞÕ¾ZË?žÓÓÐl×~?2[X&˜×?ú`%Q?|èæÌ8æn?˜!Û¿PZ?t=u¼Ò§*?—~Ø<"?qÝéÔì=B?í)ßÓBe^?¦Þ8mÐU'?›;>@³A?Œ8T|¦f?¯Äcͨì}?¢øxĄKK?íÑ
ã‡=:?¥j·ÊUP?'q…¬¼[ò?QÕfD?ª6^ðRb? h*Ý_}O?í!/œó
? š"K	Ü?™EÌãÄ?èÿÜÿ?°Áå
òm,?™½9ýiÝ?ìKqèû–?"t'^¾§?ª÷Ÿ
&1‰?O"¤†ç?°(¡56œ?‹Æ½TŽìzAGN4FGL J1540.1+8155¿ïŸÇþSO@@{w¯d:À9 *aÓY¯À<ýÎÍX
@  óS
?øÑäcÂG8?±Ò-÷ `?µk½AX@>J`vb]?ÿØ&,dŒò?ïÿµøtñD?¼(ŠbÄñ6¿Ûh1AÁkp¿Ê.ÇΏ¿ÚØ4¿¥F÷¿Ðžñ;º–AGNbll3FGL J1540.1+81551ES 1544+820?ïkrO†X¨?‹R.§?[8|TT?R-ºF7æ?Þ5!lX»?Š")wRô?ï$™S÷²?›fâ¾úÇÊ?€3 ©Ÿ?‡_/ÚF±?"SL½¤¹ÿ?'udîݒ?íÕïu:·? !¿¾'Š·?‡ã×Á¢–%?‡sŠÔC?¬¨¾ŸK?SËÌJ/Ÿ?ì&—	"?'ƒLšD?›8ºOª^Ï?|‹K\N§Y?¸Á	é¬?ÿ3@Ôn?îÐ8ȯ˜? JèlÍÅ?p,¡ø?g™;Šó¡? ùl]¹S$?Ÿe4]V?íúãzۊÍ?¬
æ8Þ·¿?'{îiÓÎâ?˜­µ×Ô
?§"ÑíÏÂ?¤îN	ŸÒH?ìÌ`Œuò?¡ðÙßn‹?Š8f÷üh€?†©öy'"Í?¶UîÁΝÜ?¡@·{èêÌ?çå[*Œà=?©ž©–ðO'?©Ñ…ïó·U?"¾_sCs¼?Éö1ÚŠø?©òé;baAGN4FGL J1540.4+6606?ìXˆùý÷+@E'8\gàÀ;	j²VÀ<'$»¡+^@,B(C–@§£áñø?Åӛˆ‡"Ÿ¿'êŸÛۑ?ÈüCŠOO@¾¦y&¥¿ã3ßá& ÿ¿âHA'O ¿êgÖX€u¿×^ä|káP¿ïÿk»9ýR¿äFù^PBcAGNbcuCRATES J1540+6605?ïäf!"?]L󍨸?P¨Õ¦Ú»?EëÜê°?cE€NWCŽ?WMD€n˜?ïÒ$}7ä?sŽhµŒn'?J¶ÜU†S·?Vóei›Œÿ?s–åÒÉå?nðö£?ïx$Ïm;?}<Bùì>ÿ?iªH¹X ?jÒ0Íqõ%?‹Œ9üÔf?yW
‡Ô.p?ïÔÉî¡ø?T¿=Ú¹o?YòS}Ù/>?BÈ+}V2?n<çÙÄà ?PªAÆÙ<?ïÈøÉCÅ?r®n7<?a~ÿç
΁?[MïH¹?rÄQÚÞ?oKÐ6Ypn?ïpYZu}—?Žëª~0l
?]eWOö?iöqŗ߽?'û\')?‹}€Ç+FW?îøñ( Ûm?‰úÜp'4?s°Èººj»?oåõTÆ\?›õ¨Ì¹?‡ 섄%í?ïsýî'Õ?v°ÅºÉ½?wf€ywd4?gAÃϺQ?‡MD.í¤?pÚMƶÍýAGN4FGL J1540.7+1449?æÄIäƒ*u@Hiˆ;£D=À:EÖL¨O?À<XÑӜʧ@äA:2@57¹«?·`éàêø¿¤$QÛ¦?×e;$C@úV6mzW?ïýÜ9QZf¿æýé¥K¿ä½`t#"¿ÞÉ«…)u¿á¾ÁqN÷µ¿é¨ü¾W7AGNbll3FGL J1540.8+14494C +14.60?âa<9?ŸÓÁu»ù?zjùÜG8?Ÿº¹Ùú?wµ~÷á´J?g·¾CWM±?ïÕ€"¾á?rî:GÞíµ?D>âN]?N†¹Ã9"?rê㧜t?p«|]Ý'?ïˆTTbz@?uEÏtGQ°?d€äöLw?kFûD5³?ˆÊ±êsPÛ?o1ŸŸ—?ï{{ÆlWä?fN¼­7s?p®¼‰½<?NB0
önB?‰¶ÿmúS?d{Ä<Ÿ‰n?ï‰ñr•ì?öµ@Kš?l
ÞIÁÃ?{\ Ìþ?†€ë¼•áÃ?rå™Ç?ït…Ï?}ö1sZ?Wå'7"¢?a‰ØÎé'»?°õá&?âS¢u~?ïdͪ?‰–ó»½Ê•?qwß%8‹?t &¢Œ?š>[°Tñõ?…Aˑ\?î{¤5Ì7?ƒFß)?‡·ØÙQhÉ?m ³lͱ?¢a…rû]?'xÅÿH3AGN4FGL J1541.7+1413?ÁmK®\ë@H,ü'œýÒÀ:ψ[ƒ´À<€©={‹'@ Œ«hy7?ý|=¸ƒj?Ë6¢Êê?¼»HjýÏÏ?òÆ.jÑ@ÐØ;Y¿â¸J^Èã3?ïôhAÝÅî¿à@ÝݖI¿ÛÜ\AŸ\§¿Ý`½¨"¿ã6«ÃgÉ=AGNbll3FGL J1541.6+1414WISE J154150.09+141437.6?ï¸ÖSðSK?šþ{ýn®ž?@²˜Í"úí?M&(˜
S?€¿A€GGñ?šf\Ûl/¦?ïԃÈÕyø?r *LŽÜ?HlêÚË»!?RÀ´¾H²š?r°~ZGwú?n"ƒ–ª&\?ïŽÛqø<?p+nüÆ?Z‹\@"ÿç?C»+4Ìñ)?ˆ÷·ÿW°ã?nVù4Tˆ?ï1±¶Ïh?melì<~¶?u"súÐú…?U~KЅ~?",$\?l
Š#ÿ<w?ïœè#rÿZ?•sôñ
†Â?Qƒ4=ƒË?Zwö ‰?†••H¿?"è£dm?ïr÷ƒQ%.?‰ÁÐeÎÙ?`UýüÝC?ee›½nª?Aɬs.?†Æ²pCù™?ï#1ÁÕ34?'û°Æ¢r?d^Hô/N7?R(]hÒ+¥?™
þ£è¿?ÏÒêÁ%?î§FÞê9?‡è+R25?"#+FáV?nbüK*ûË?ª|À¿Õç?‡"Ì"(ý‹AGN4FGL J1541.9-2915¿íLnČj@4c†Â&€À:ŸBP©À<3bàŸèh@ h ¢¢V×?ýRÎ8ݗ?¹íY	[ža?¹+œïÑà@¼íƒüyc@°|OG'?ïæ'P¡Ù¿ÖWÀü_©¿Ë߬bôìÑ¿Ôè#ëA­¿âüæÛkÌ¿Ù78+>AGNbcuNVSS J154203-291509?ïµÎéàÀ?o3M©™?R"°»°¡?=›äÕ&å¢?€9é|Ñ!ô?mÑ
ƘÛM?ïI5c95V?ü+LC]?wz"¶Ìšú?y²´»è‡Á?ú²c?"?‰¼~IQŪ?ïkà)\+
?väف»ªY?e[+°sÄ?]oK¿ª{?±*Õ¢¦Œ?ttòÝ6F?í&‹ÂÁ[*?ƒøÈëw ?'¸îA¾F?m»kbc÷E?²Có®Òª¡?à3ÿŠ‡?ïk©=ÑÙ?'ܦ,y®‹?iO^þ	P?ZÒJƒe‰t?ŽÑÈÙ#ýs?×R10?îIÞ«O,?§wÛUgÖ?‡3lï
?«i&"|??¥¦:ë1"?¢ØÚYú³•?ò–Ô?¬?6í??tì%|9O?nxW'¾b?¡¸'S÷'?ŒdíúË·?èצ>1'É?»x·Wã?¥"Zù׺?‡3¡i²ü?ÇXÇ0D…/?›†.Öø¸AGN4FGL J1542.3+1801¿å^ÉÌ3Â@HÜ#|ÜÊqÀ:¦µ{wo£À<\š¨Rc@ù¦&oÖ@ ,ƒɖ?ËhO_8Ê¢?Ïÿâù´âJ?þ‹¾z#²@	Öv·Au@¿ãµ>p~]¿Ùãàd¯,¿èh‰ø;æ¿éç§^~:™¿îRËI?3¿ïÿ2FÄàAGNfsrqOR 167?ïÔð(,Ö?e¦¿Lñä?ZãsüRÖ¥?M'ºW
ä?mžæބz?a5rT½Õ?ïšJ÷u?ŒC"¾ä7ë?c²Çh`ô?gX´Fûo?"‰~F Ü?ŠFÊÉû&Ë?ïve/>ö?û˜ ç?svyTçÐ??r½‡ò"'ã?ˆ«wsœ2e?y–!òÈyÌ?ï60>>ݔ?rJŽ•ÃÄæ?€m¬p?^§°Zë§?'+Ab¦r?oª¤á°c?ï¡Æ¨˾?yù±ù·ƒ?iK&*ŸX{?d½|-;7:?;Œu%:\?t?%Ÿ–Ǥ?îÊh õ¥Ö?¢Í0·è@?uR?'íÑ?y‡–ÔA²? ¯$Gí[a?¡Û®1Ä,Ç?ïtFŠG?Š€–Ãoc¸?~Äà˜|PB?z­X¢µJ?—@?
Vðþ?"¶Î-«ü÷?íše4?Ö7?"ë­è¶+?—Ud!F?€Íîâ؜?ª®ú})äd?"'OˆAGN4FGL J1543.0+6130?Úyi†_Ö@F°üø
Ã7À7‹g‰|$À;LãGb•!@ Ï6K?þdØâ"Äö?•#VØe˜?®vý@Ã@•B½ò%@
˜™êL¿¬"'È¿ÙK'àD£É¿ß´`¥_@¿Þ–ÖZ²Ô¿âÌdȵ2¿åcܺí§AGNbll3FGL J1542.9+6129GB6 J1542+6129?ïíÒÎÄt?R<Coì\?6±z·Ë´?2ã)7y´Õ?`ýÃqz³?P-}=w ?+<n?—ÌÙ8]?a«
ߜÓ?kÊ-ÜïF*?Š3òŒ)7•?–Ïr™zé?ïªe¦šUy?†?™˜Îá?iØ
×3¤?x¼¢å Ø?}á'6͉ó?ÄlVl¤?ïÄÐ(ÌÓ?aª}ä$¶Ò?V¹h"Õ›ç?A?æ2R·ë?xN=Îã??_²î+Д?ïêûó@U?X*°ÇÏ].?1ªÁLúy??(!GÃûýC?bδ " ?W]~úH?îÜÙiŠª‹?¡œ"'J±O?rtö³æJò?ƒ™×iú=Ë?ŸÇ•(¼Nà? AH>›Ù?ï¥Hüôø?ˆzìyH<ñ?g2—s+ä?yßƒ'/?€á÷Òò?…ZYÍ,ÂL?ï…	庍
?yƒ'(ü?d¶ñk*,?Vçp'2†~?‰Ê=sÁ?wOPÑ¥ãÎAGN4FGL J1543.6+0452?î™HôÄL@E¯àŠï²«À9ð³!*3À<,œ \–Ú@ {ç_u0"?üxœ‰8#?¼W®'¥¹?²á°^­	Ž?ù(¤Ð.@
nòÿ'p*?à8Q_îýú¿è*<´¼4Ï¿áÄö¿w'¿Ô¤Vg®æ¿Ý˅å\»˜¿ßÚD.®AGNagn3FGL J1543.5+0451CGCG 050-083?ïøÍp®
a?5}[KQ™'?"­Ê›Ÿ¤:?ªXlœ	?HÊÖB?2ë"ÌÈ2¾?ïޗ
Ú4Ð?p'jQ~_?@kC´)V‡?IQÈDB"Û?mN$Náˆõ?k̳³"?ï¾~s	³?pf	³ô?OY-wK?:	Á½fB[?|Õ ƒŠ7ù?oÿ¤[+¯7?ïvrèÕÁé?gÅeÖų?a4äªG?@ÅJ?Èј?ŽÕÓ?fq°® r??ïõ,F§P´?Bí»¶Ædš?0IÖÓL/?6`Ã<3
?Q"ý`
ï?@Ò°¸œ½ú?vÒg?ˆ»R¬R?UîçáÊ?\´ndh0ª?Š[rã'?†sÊÍÐ@?—Å.?w}N@Êy?X•=8´Ö?Ha²Ö"dT?Š÷ã3å?vÀÞ¯Øb?î‡é=Q‰?ƒt(l÷K?u¾''–l?_åe'&ì?¤Éªì=$?ƒ(¶—`ïAGN4FGL J1544.3-0649?îÁ¢(Ö°H@BŸ¸gÀ9%'œüûiÀ;њ#,Tó@ 1ݘL¦?üðI ]?®ÎdÒg–g?«i¾_¡¦-?ÿAVâdå@Nn|4"?ïñâÀÿäý¿Ç=ÈwþiR¿ÙŸ¹Ù«¡¿Û R:µ]š¿àÔ7ŸÔq1¿ÔåÓc¿ÂùAGNbcuNVSS J154419-064913?ïú›ù£Î?5¿™©º?'žâm'o?
µBÔ
t?D{=aâ?3Äöi©;ù?ïé:'‰k?h¡²2eڅ?4ӑö"P?C¹ªœ#t?d+t_'Í«?e°†×8?ï£ÈŒÿµá?v÷šB™R+?_xn&ÕQ?b Š•îßß?ƒí¬vW)?s6à|+?ïöܾ9ƒ?7ã^Bµ4?ä§'9B}>ú©Ó«®"?Q9''tìÑ?7}›ºÞ¦?ïù£PìE}?=ã\ÑZ	š?!°©XM?(9æ.»?E'ÉÏJ?:ˈN¢‹??ﴚL$¤X?'Q´UO?MJ|³10‡?YP¼ÕKµ?Å8:Ã?€£`àõª?ïnåîSQ®?…*OË•Ð?f
fQ•äK?k›(òàÛ>?ŽÃêʍz?ƒ
äuÊ*?ïé¢ç²<?VQóVë?#V§¦¼L?³È'Ç?e'­ä?]K?U¦@²©á<AGN4FGL J1545.8-2336?ځ¹T0?@8ðgȗÀ:äì-»$.À<a`'÷–¥@"Xײƒö?øpDÖÉ¥Ñ?ў@}·÷?Æþ<"¿j?óYæ/tb@3Z™©‰Ò?Ð0ÿV·È¿í¢FF5nw¿âJßO0j¿¼R—|ˆç›¿×,àÞ§•±¿åï!öÊÍAGNbllNVSS J154546-233929?îØ{Zz†?œý#ÙX^V?`¶pF9wQ?Whý`»œ?¡lãS"È?œŒ=n(?ïp;[³;?'lšÚwµb?gNoŠã"…?nmáÖYs{?ŽiŽ
?7"ð+Yr?îÌғF?'(ììÑ?ch ¶ÃX?f©áRzR*?¢	ÚI¶M?'Û'òa?í»³öÎ9E?Œ²Èy1îZ?kȉo¥È?TíŠLÁ™ÿ?±DüŸs.?Œj×Tß,*?í9Nš¿?²Ð—3m'¼?o†$™«?a֘çcÅ+?¶Rh´8E?²˜õ-3×Ø?î WÇDÖ&?¤F.áµ?uÑwföÓ?'NzI{í?£XéZ‰ÿÂ?¢Pz.ìB?í®)"ÄÜ?£)‹%ÎËÉ?p†T=§ÿÜ?pI‡9Åö{?¶r)q36?¢úÞÄK<ø?é{n^ž?¦%{L˜B?|ù¶½$cç?rš
ýµs?É*z:aXh?¦ïmË/AGN4FGL J1546.0+0819¿ÝÇ àö$Š@FVV>Ðö'À9¸ÀûÞ2PÀ<)µÆ 
b@×-¹÷ˆ?ü¢HåL"?¶íz—JßÍ?ºÀ‹J÷J$@J˜Yþy@…Éy±ì¿äz-ô/¿âDx4Å«¿ÜYˆœò®¿Ð™:¤É¿ã*T'8T¿ÞÊ^=M'AGNbll3FGL J1546.0+0818RX J1546.0+0819?ïÆ;6—š?ªf%ª²¼B?NÓÈnþ…±?{€r¡s/à?yëë Îð?¦ö»c¼êŒ?ɨÏ?3矟4¿?b€7¥`/Á?eäè#ù°	?ƒ0¿·¤À>?{"-'ó?ïz:JËø‰?x"èô?dQÏj0×V?VòO–ªÍ?Œ\ùd·8?vI³~ýI?î:ŒÎZ?zÚâš°*?ˆo]"Hhõ?e‡þDžªw?¦Boçôl?w¯á'S??lÖñ?sHáç*aù?U·ɞ[)?MgÀ"D¿?|xUW~?pvH؊'?îυVkœ†?šO¤l¬1¿?y«²v1¥?ÔÏÞû§™?Ÿ¤ÍÕüÅ?•<'=Àç?îô¸†Tÿ?‰Ûô'Ç©©?sY cB?kP4˹§V?œ¼'…˔?†Ÿ#Ü!?ë'#Ÿ[>?–g1ˆ%b?œ\
TÎÏ·?'¼Œã¨±?¼Xˌõ‹!?"A¾Ï#¸AGN4FGL J1546.1-1003?í"Y`ÛÒ@@Ó£"¯WqÀ:°ÐíÄÀ<1Y²"ý[@ bû0bsh?üqÖ¤?Â&ÂaŽæ7?ÄG0€¦Xš@ú¡ÿ™¨³@\ބ\?ït7àAØ¿Ùñã݊Š2¿ß^¡Ëí)¿Ô¤ô^N¿à½çŒk³­¿ã4…
š¶AGNbllPMN J1546-1003?ïÚ`"r?ªÐµ}m?k¶â¬n"?ª×o¾Ùãï?SÑõðKpÛ?FN^6Ù¾?ï㊁¬E¡?m"[;¸Üa?@§–YƒÚ?J[?Ž>bö?hp'ÒS?h"/Q/W?ïµY¸"B?nk3H
"†?WV݂â¨î?FOºèÀá¼?j›ÒËhÅ?l3‰:È?ï¤òÛª5H?bhsÓ£?Uæ€8b?7ëÐúûGÐ?"Œ?Bzï?a]+…q?ïè
 Ñm?Ž,ґŸß‹?Y"ô¡Ëò?Ž/"Çw?VfÉ?¨ý/?I3©Á(*¡?諸þó­?'·".Ä\?QÑëD²«?]䩤´îÊ?ƒÕÖ_j?€ºùëZØÇ?ï|õ èA?~dv´S»?d£IÌÌÔ´?aé,!n¬/?‹™Å'Ù¬?{LÊ\§Å?ïfϗØN?~1®"}tÀ?j'Ùÿ?V3ñdªÑ/?œA#˜p?}$³"AGN4FGL J1546.5+1816?Åþ"Ënæ@Ho"5ÒIäÀ;¦¸¦¥À<€rmæ@û•b'g@š¸–ž=?ÊçæٓZ?Ä2õö'Â5?ö+—]7@úx3ÃPø?ÂË>Ø,ý¿ÛeEÔö¿ÒZGòÝÙ¿ê\žÊù¿ÖäHŸ+(ù¿ïÿ×ñÃýAGNbll3FGL J1546.6+1812MG1 J154628+1817?ïBËañ?Q?'…Ušž?vÒªpý$K?‡rF97h©?'ñé%˜ÌÝ?‰½uWJ2·?Þ
?|ٙ%+?X*kàåÔ?[BÍò÷	à?"0¼éÞ^?zv|'3UÖ?ïJfÂï?	"é»ý;?mÝÏÓaA\?m¬ÓŨØß?'÷m¿‰õ?~UŒŠûŽ²?ï>,š=?q8ŠOï•p?kZë^_h:?So¢'û?"ϱ}c?p¶/'ñ#?îYÚao
?™ñÍ2.mª?'»uûÆ?"Mwló?¥³|¥µ4>?–Òé3š=,?îüèGôا?–pª£È½?l½jÞ3A?s§"÷àU?œËI«Iä2?")gí?îvTÁ+¥?'y—©Q?€xõâ~:?~ô½Çí?¤|vwog?ŽÏï˜^?í¢
hjÄç?'
7ËÐ à?€¼"Bée?qr®ß#d?°ØjÐkX?gÂF½ÑAGN4FGL J1547.3-1531?Ã;x,©@=¬€ù£wÀ:ÛºÌð;À<kx(/Éò@!&öÝÂhp?ûTÙý6ø?Ô<Iý·{?Áõ:i³Lô?ò'r…X™õ?ù4Í\i¸U?ä¡ìï'{?çJ{NTø¿ßõ¯¯…")¿äÛî=_Üß?ÅGõâ𥚿åTh!§o›AGNbcuNVSS J154725-153236?ïY~/»ã?†nH²÷8±?VÔ,ðªsÆ?GB{z÷¤[?"bëKÍd?…ôCޗE?ïLf崜¢?™3:…†?p8Rà˜I?të<Q?'eø#á³?–õjÈS?îí~âÍÙ×?©d—0?oq87»x?n®	äíl`?žaü˜n*¾?‹jº¤zIý?í™\_§Zw?)ŸQ7¬Ê?xgµ:ó½›?j–{0+?±®¡°Â¿©?ŽÑ²|Z?îH‹‹>›?ž¬šÛ?n¤&«ßn?aü©"ÙN'?©åío?ÏC"!E?îg··ðOf?§ÿò}±=?€«ªKÄ'Ð?ŒÇDµ'&?¥Y™éêwª?¢Ï¸;OŸ@?í›Ø¨o—µ?œ©Ý,Ãì?|¾È"|*k?w%8M–7B?±UN<kC¯?šùãÈÒO?é²:–n}?§™5™˜?ƒélóÏÂ4?µI'ˆ?Çø(¦?§5L†ÅAGN4FGL J1547.3-2802¿Çôµ7ô|Ù@4‹eˆUÀ:FäH•À<?,˜@ ¬Ùuҕ?ý¡ËFºÏt?½#Ë6I¾? ›_æ?æ̆'ø?øC®®(ÇÊ?îÎQfúàÜ¿Û'\:h‡¿áê9Ÿˆñ׿ÜÛÞaÔ¿ßS…
EŽ¿¿½¿¾œ]nAGNbll3FGL J1547.1-28011RXS J154711.8-280222?ŒyÔ
?y˜,÷ÏÃÄ?Tß´úîx?DyöÇþf?‰ºf^Qñš?xD$+LÓ?îõÞ§Hav?œ6w™Fö?~«w£¶º"?‡GîêK"?™™M-*;°?™Š2ž?ïAñá‡ð?«Ä?è©É?pÏò?¦Ê·?q
3Ììpl?"ßðù¤]?}¢Ü^ö:›?ì@¯,JX5?Œ²>…"?"­"ëðÝ?q¨'OŠA6?¸Ï=â±?‹Qbb¬°?ï.È`½–4?†ù"™œ™Š?g–ž^é?VŽë1w‰?—41;àv?…vŸÚÖnÅ?í$&ƒ€R?³¼†ÜèÂ?"MØË¿£È?™{HJÇy|?²U²YÇ?±‰wŽÊ;?î–qCd-Ò?ë'Ó+!?|LºÖóœ»?x¥#E–kt?£TmÖÍK?Šþ]'Ì2Ø?æ.ñÒb/?¡¥EÐCÚ?§4Áí(á?Ž»)ø|?Ͼó
9‹?¡êÖ~û~SAGN4FGL J1547.9-6403?í¡³ßɇQÀþã'áïtÀ:†ƒ<`À;Å%ƺd@ò·É°b´@ßå®E"?Î
èuõ¥‰?Òþ¥¢fqÏ@ˆêb		"@ƒ&uµŽÃ?ï·Do›™N¿ã~Qª¿_¿ì&×¥mã2¿ãlja=1º¿ëcՒn,.¿ïþ|AGNbcuPMN J1548-6401?慓ªí)?Âs$¼ð-G?¤â$ç"ÍÉ?›L؝Pãf?ÐX"
5+?ÁĜ{?äÕqy?%?Å`¢¢V×}?¤0X…¤°~? \€]®=?ÓÏüèچ?ÄczzçÊ!?åm/—·)?²²½Åp?µ,<JP^§?¢háízª1?ϵ#| ©G?®×;ÃS?èøE«|?™¥*H2[¸?¶5\VÃ\?ã÷›3uï?ÁìÁèJà?"—6Þ?ÛøõŽ{È?Å´¯oš ?¸:ÄôêŒÌ?®ítFª²'?ÝøY4œ[?ÆSÇsFŸ?×D@ˆ
?ɗ+wŸk7?ºLÈ»üp?¹•ý,Ÿ?áß$ym?ˍ?Ñ.å?ÝÜQŒ\Ä?³ú|Ä÷'?´jQÓS?©G·ËDÌ?ØÉyK…'?²Ñt_Œþ7?ÞéÜkêùw?¨=¹…¥?Ë·©"c†?©ÖÌÛ
?Ó:OÔÆ?¨Æ,òÚèMIXED4FGL J1548.3+6615?ïòä­$w@E0å£]gºÀ;—¸`.>À<Çç˜*-Ñ@bÿ"	•*@árƒ«Ë?Ãà|-Q¿·H"ø¦?ñrרÈá†@Kžuvy¯¿½;~0\"¿á³—!U<¿ë»G¿1X¾¿œ
F}Ë¿ïÿ¬ž5¿?ïýÝ`˜ÇAGNbcuNVSS J154831+661632?ïCQ
Ž´?¶,ð`¶à?z£®q8ÿ?†Àš¤o?–îª;TM?µ'˜BêPå?ïl×áʌ?–I
?pšQ]ìH?|	Ýç¸É¨?Œ|ßF4Í?ˆSÁ¶'˟?í…ümp¾?¢üÁ‡lÓ?'úïÑ>]?…\´–:?±wâ<Z*A?¡³Fú÷h¾?ï"Pê~8•?r™g6ôH?lãIˆV"?[Ñr'' ?ƒ²òô
_b?o=YÏ"?îû"V´l¯?£ó*ÔpÙR?ŠØ°Ycä?úžä~'£?"!<÷¾N@?Ÿ_¹¬'"`?î'IA£Ÿ"?¨!]@ú{o?F'7‡˜?'E…»ÙD?¢‰ÇgÓ»ä?¢ŽœÊ]?ìJvf
Ðù?ª•ƒÚšµ?"ù‰Q–ô?…*•É¹¦?»
¤ÿ±Ú?©¿®²(³]?î#ûw°Ó?—Ë•rÌ?'8ŠTé?‰A݆]›Ÿ?¤¶,''
c?'ÑՕá7ÅAGN4FGL J1548.3+1456?ëÀ0'¡?ç@G˜–gµñ¿À8ú‡Š£\'À;É>»ýq°@'gh™ò?þ¼#1]p?¨FΤs?ºäÄæ#Šõ@uâXOL@Ý\ª%?ÞÏh=V!Ë¿»N®ä¯l•¿ÞSa;":¿áDÑöØ9¿ã^[`m~¿åÁ‰¢«'AGNbll3FGL J1548.4+1455NVSS J154824+145702?ïöïvV/?DoõìÜÝ?7)Vvz?1Íy$:Ã?L-NäKS?>·ž–'ñC?ïÂ{åvg?tK¦ö',?Sê×Ä^?X\ގ$uG?yÞ—ù°¬?p]éçþ'?!ž¾Ð?…°âvÝK?s'=€ýO?~Ê%kµ?€À˜è>?|"Râ—æ™?ïŠ&œCd{?f±î$Ù?jõeÒ×¥±?M&fìY÷ù?†¸ÿlZ'ß?cxøº"pª?ïï=Ýܽ?SÎ|Ó¤Ó?=Y-ÐEû†?4£ÃÚrY­?Z-øXè3¼?Q6ýzN?ïB—Í¿k?"?ÛæÐ?hžì¼ñ«[?xE"W(h?"™(Í­.?'F°"ñD?ïxzÀ?Š»µ1×fÏ?x½gì~?'Q"—•=?…ŸmÕ+Ò'?'9^Íîx?îþ˜ j%/?É3ÀïÅZ?zçVƒê?bÄ»áçj?™s&L̵›?€"l*{^AGN4FGL J1548.8-2250¿ä—´¨@8,Â?«ºÀ9vh<)|À;ÀŒÒá¹Ä@ â×býÑ'?üâh?"z?¬Ï˜ü]* ?£'£Ÿæ?÷«&[´@
6¼ÕˆÞ?ïÿû-2h2¿Ì—Û´q6¿ÑWå.Ãaê¿Ù¥"Ï7á¿Üêö¦""¿Ô΄þ"?AGNbll3FGL J1548.8-2250PMN J1548-2251?ï⥮½ç?f:zZP?'×òà	?7ù>k7ž?kÜғ],è?eÀÚé)«ž?ïÔ﫞ÿµ?vÖñF$º?LK¸{è?Vîv'óÖ?qþÈÙ?rÊGÌô@(?îÞà¬cÜÚ?–Y}v'¦)?g—ÕÈ­±?r	.M€ql? ˜ƒŸ%Wz?–[ó¨ƒÂ?îo¿—w3?"ˆØa™Ž?v^"Sí9•?SaG«Ø»ä?¦8=›I ?€…z!]¡?ïÀæÜ\P¨?zù¤}—•?8?±«7å?2þ»†ý(k?~ ±:ÿ?y¤HNÄMh?uu?‹Ÿ&Wtß?^‡Y,U?hãF@–!?Š»¥]i9?‡cWƒÃ›*?om²F?™0æíW?h,"õW÷?rô»÷èz?¤¡pìeê!?˜GVh²êû?ì2tÇÛ©è?›–õÞ«Ÿ?‰iñs:ÙG?oOcќÑn?»?–*ñ"?š~zž¡†AGN4FGL J1549.0+7846?î¦p8'ä@Ahšþ§±À;çÿ:bËÀ=&(
á'@ ®ëA'v?ÿ³ø`îW?у¤D˜`_?"†`ƃ u?¼|`"Õm@¨ÊÈ»›!?ì¼]\Òi¿å­½Þ€i¿×¾¤kÚ¿Û逢&Ûâ¿ã;ýÂ8T¿Ø;Ä~AGNbcuNVSS J154837+784526?ïèÝÿÐe?Zxým ¤?6ÇVÀH(µ?-z8eä†?dIe÷d~?XU"N*?ïÇÚÝ[»=?vº7§iÄr?FñSÍ`èú?M¤ÿ£øk·?y4f¼[K?u-Ø¥zý½?ï?çyÔàË?Šs©sk?qMTws¥y?}z8ö)´"?"¯»«"";?†.4ØUÀ?ï×mbPz?YÍíös}?FS…+"µC?,,æÖà?q¬XÄUoŸ?Y†à§¶ò?ïÌp'/Uê?}‰p˹a?C쾟<U?@q.ô²T?wJ&ôôNÀ?}->k7?ïu幜ˆ%?cË^ê¶?T~ïîè9?a§ÃŽl¸8?öφŽÅ˜?‹	ÖÊOå‰?î'ùrOÜ??"ÄBPÏû?qùyUçË#?|r"Ûë~ä?¤'9®åj¯?")É÷;–?ïv¡¡>ÃN?xü¬Ƹ˜?ZV@čX"?L۟Ť?ϝìÍd?yFãþeuÏAGN4FGL J1549.3+6310¿ìZ")=@Eô<³åuÀ;NÊW§†ÂÀ<f<Àz®ó@Àe©}y@>Ü´¡]?»^ò>Kj7¿Â¦jŽ.@ô<¥¢¼X@¯:¥ÃH•¿ÖúüDÿìaðµà!=¿æô'¢TS>¿Ñ£ÌB¹8¿å€|ý ¿Ý¸ƒÕ6oAGNbll3FGL J1549.0+6309WN B1549+6319?ïŸV¾8ñt?ž''-s)
?[1NZÄ>?"&÷(&¢õ?"Ä&´?zN?œÖñIöòz?ï—Tû"ñ?"êm‰ø?lÑnÒF€?‹šk•i"?'öekwnã?'™Ïw‰'Ó?ïhÇÎ¥ó?‰ãy/Ãql?Y¨A<Á•?dÌ6§?u:?'L"ñtŒ?‰`\Ô?ïý«^_~?t훦ȁé?TĹ)Ó?Hÿê÷µš?‰'þ£?s›Nù­îu?ïċ+±xw?~ü"ã?W¾HÔõÛ?ZÁrÀk¼?wú:•¾rá?|~öˆcŽ?îú7Ìu? ÜO|¹á?t»ŸŠ'{?‰ÀkžV?›Š±®Ô¸?šN#m{*?îãd…Þ?'kjén?eüW‹K‡ò?kÖRˆ"2Ú? núPìì"?''–+â9?î
j(è¬|?œÍÞÑ7k?}b~o¬'?zˆ¼Ë?«}
 ;D0?š}ž-«s‡AGN4FGL J1549.3+4234?ÞAôuÌú‰@IsŸ©~+À;Z|Tå5À<ì¿\¢˜@awcä«ç?ÿÛãõhÍ?ɘÂçÇ?¿^Ðߚɉ?öH8c܊@\­+qÈÅ¿ï§î'‡Ù?ïýk›Y:¿â™ÝW‰¿ål妸f
¿Ë.×XìÖ-¿ì¨Ä¯ÇÙAGNbcuSDSS J154918.64+423500.6?ïÃkÓ?mÿOuC?R
zˁ×ß?Fz {$T?yÇÞÕÓ¦š?k8Ee°Î?ïҒct?q·›Xÿª)?IZÕ7?Q±'®.ví?s‹˜
>ä?mxïf'ù?ï`$*VÀ¬?}ß,‡²»?cµ2""j?^W
ܲ‡ú?'"Ôc嚳?zï¼ÚÊ
?ï®e)ê#?b¯IH¼9?e쥄-Q•?Qž¨>#"p?}×+û€?`"}íÂîÙ?ïj³yXuQ?ƒa&+]?m5[7Nm?d63ÿpþ?ïTJÕÈ;?'Mœùôñ?ïneŠ&?H—H†?_¯´¤%ü?gTv?—Y?8S\7¹?‰k¥:m¬Y?îÄ©£ä‹?Šßà^\Ô?qÏQ£à?jönn±…?¡'«Ý¡­Ñ?ˆl±éx}`?ïfêð¤?€33BQ{?xëçœkë?o×Y˜J­¯?–2ùb¾!u?|³	}½PAGN4FGL J1549.4+7409¿àâð7–P@BÜÿ—$tTÀ:¾‹ƒVa6À<±òeÊ@ Œ7Ü:S@EÖٖë?ºw¼úò¥¿®sìôQ?òæY¶T»C?ûn3´ãL¿Ù¢¥œ\AŸ¿åü†™Õ ¿êŠwB+ɇ¿ÒײÄbðæ¿ééâ‡I4ý¿ïþS!æÕAGNbcu3FGL J1550.3+7409WB J1549+7409?ïÈG+…e?q0Ó
Â9?b¯¦Ø8¿#?Wgq2X&?r"–Øí"?l9îë[j?ït>&	Â?ËXEû?q¿&üÛ¿?~ŒÈ]Kêu?Šâð2?'‰ÄØî3q?ïô	k}k?‰ùÎrLþ?<ödM—ð?Øð‹¸Ç?–c¦á•?"ÀI[¾—«?ïHŸ}M!‹?v™Í/kþ?ˆÜ¶ŸšØ?q;\íTÎW?…JCò¨f'?gOðɯ?ïmÙ	F$Ò?"ÉމLjH?{ñ÷ý?ržâ	É"5?†Â9Þ¹'?	bÜú?ú+2f?¢Ïÿ‰²)?†k¶ÔµEê?'b•Bê,Ñ?¡»Â¨ûo?™[HŸ,àÇ?î^9÷r'Å?–³bK,VÔ?Œy‡Ý¬d?‡Í8?}¥?¢ýþ¤Ÿ?':f"oÊ?íj†E¡AP?œ¹Ä1r¾¹?¨¤yh@?˜º#œ? ³"<!
À?ˆ9n'WNAGN4FGL J1549.5+0236¿Ãèõ] Ö@DqÔbÃC·À9%[ÚjÀ;ümd‡i@ôÊöˆÞ@òÁmóùb?«ÂÑBÊ¢H?®Ú€Mœ@háa«@¯CWË[¿Õê0_ï(í¿å@ß=è˜Û¿ä¢i÷ë_¿äȖ<"¿ë´	tC¿ïúÓÍ$áAGNfsrq3FGL J1549.4+0237PKS 1546+027?ïâ̪ã?\6]ØÍßæ?DͲûVÈ?2OLÞýœ?h-¢©g•?Z…
Û´Àí?ïÖ-í+Æ?o£v"4Ç?G7úãˆ""?QYzË[Ý?ri¥å4?jhB»¼±-?ïŒý t7?…2òuÇ»?cÿN%96ä?i å,Yð?‡Àä\ž€?ƒn/ÛªS-?ïìZ¢Ÿ
?DªÑ
Çéa?FŤµÄ!?/îàó–w‹?[çèc®‰–?@cjhâ$?ᅴá>ì?r§VGJ-?T'¡÷Aۏ?Eω)±Â—?{
fȜsŒ?q?\PÖ¹¸?ï~ÕnÃu?'·Áµ²øè?V")Z&˜?d‡×Íò?z8¦ûÝ?…¿ìâÝ?ïÔ¯‰ì?"õ\Ôet-?q±9¥"yü?v40@µí?˜Ù¬Ý,ç?"–b¾¢MÙ?ï̀ŽÛ¥ƒ?dÝeóc2T?_Õä($?Phší…jÀ?qÊ?i yÎ?`lí-[SAGN4FGL J1549.6+1710¿êxšà@Gä\ÈWóÀ;%–'~À<"íٌÏ@½³Wô†@'T·?ÁlIªC
¿¤ú [Ùß?åQ‡F°¾y@— t>Á1¿¶|n¨°¿èÀ*'_–>¿ãÐÂOpV¿å2Át‰À¿ÝËŸŠtc¿¯Öa"iAGNbll3FGL J1549.5+1709MG1 J154930+1708?ïë>2%þ?Tƒ%ú¾Š-?<'
Ž.Æ`?+ßfÀ2^â?`ÞâZ÷?Rò)Iµ?ïŒcøÖt?s븉k?FŸX߶?O8Tbšõæ?zbâì}{?r6&áð4?ï• –¬
?æ®úáÚ?SKI¾Ã?>+TqðÊ?ˆNqß,h?Ì 7T–_?ï¶l¶ëÂ?a»­å³Ó?E02Â×?,	0ÅÄ`?Ï		ã\?a7ðáAâm?ï¸JtËâu?óä˜5`s?P~	îZÙó?Aò{̗´?»C×ç(?§¤è`àÃ?ïXrrí?'ø•ª+.?Uñ²"'';?a¬.º--û?"£Õ·Ëì?'CªKXô?ï;˜?…¾?‡»ؤÆ?^¯S)œ«M?[G
rÙ	?–¢ܙ‹?‡ešëQ'Ý?îáê('fv?"RòïYA?bW?ô	G?RÃÏvki? »éÔÚ4?"gÒhqAGN4FGL J1549.8-3044¿ïâ"Ú#2Æ@2' d#–À:§$WÎ/À<h;¤ñ¼p@!"ƒZ=
?ûñLÞÕãÍ?Å/âç¸?¾l͞-ýê?ûŽÍ=5µ@f?˜ò)Ô¿¨è7Œ^H?ï³!ž¶9¿â[ˆAWŽ1¿Ò‰ÞÛÃ	Õ¿ÕJҌ)nŽ¿å-4±B-AGNbcu3FGL J1549.9-3044NVSS J154946-304501?ï5 Üë?z
"Z€N¤?Wq¸næÑ|?K	x›Wi?‰`¶îH?xXÿ¡'"Õ?ïŒÊø—÷?Œ ÜfÅGM?b·²"4¶?gñf.eª?ˆU‰3á?‰€&oL?ï3ôŒ%à?‡éö«J?cD7ªu»Â?_•fiKŠ ?—5zv˜×‹?‡ö×:΃?íáÅçD6*?…Ÿ%´?nG?†R-°x"x?hÁµ"QZ±?¬OæªJ?…ÇÕWþ?ïš-éd?'Otü9™?sñÑ9©$?qûŽSÜËC?šPEöUó'?î4Ó%¿H?âB•?¢']56Ùá?zJ0cC ?ƒ¡Ã/O? »!5§#<? ž=¥i?î;õÙ²?—>‰ªÓ?oY(bç*B?e@êÛõl{?ªKŒlm8?—$8Æ$z?êœY	†'?Ÿ)°¨~ä·?™1橃 Ð?†©›õ]rs?Âh_Gbj?ÁlEQAGN4FGL J1549.8-0659?ÕÌVÎݍ@A}j@ºˆÀ9=+úYÍÒÀ;ç<³åu:@ÄO(1L~?þ­ÛÛ]‰H?®ªq>lÞa?':Ǭ?ðÄ öð@¦®<éÀN?ï] Å¿Úó)âÙ¿âŸÒ}浬¿ÝT]¥L«)¿ÛÒ_qÕÛ¿Ú@ŽERš'AGNbll3FGL J1549.7-0658NVSS J154952-065907?ïÀÎì"¢?oYÅîy?QY³šâ?CL&'g°Ž?{BÏ«cÅ?lRú"˜?ïÑ&eðIÕ?tæ4TÉT?Mä†@.c?V›N]WµN?s°<W!	?pv"ÍP,?ï}>‰uª?{Ú^¿€Än?bv(Í?XR§ ?Œ+€~
w?yœ¨ÙYÎU?îÛð×*C?wU)â»?}\{îCX/?YÇÎUè?*Æ#ћˆ?t5æ,v*?Ÿ3Ü?'õ°Pô?_øšâÃ#ï?Q'O}Š¨?ŠÜ«¤?€¿D?×Æ?ï|ÿ"=N?‹Ÿ‰ä£©?aœOãmÓ?lªÝª(³?ŒY#tÞ«?†æ à::?îünUs$?Ž¢z{ù?o:ŒÍ¿??m»çþ?œŠã¹Çc6?Œ'àÔ«?í6æ["%f?©¢=Û?'
I4Ed¶?tÀ6î²a?±Æ:Õ߈ ?j`FÛoAGN4FGL J1550.7+7006¿á6ãÝÆ«\@DjËGÀ;@öý»'À<º7ŽÆÞ@<Ÿg™?ò9ìxkL?ÛtiÉÈ5Ž?ïþMþ"7@O×^ FÇ@úL+&Ê?î¶Q•ôÉk¿Ýä©ÍÄC'¿âèj{€)¿ïg/ò?M¿ïŠÿ…†½¿à(6îÎAGNbcu4C +70.18?î|œ÷Ù&3?¨}ódªé<?xŽjä"Ýz?~ö
ɵ¨²?¥$c':Ù$?¦½S¯•ßo?ëÊcw.ñÁ?Ä4Ç¼JQ?²¶äó9?¾Ž½-Ú?­í¦¿¥z?µŽü'×?욐â2\?£Ã‰xƒ,?¡-ËÑ`kŒ?"㱘/Ó?²""t·?ŸŠé†›)?ëÛ&™—Q?©sϬ6e~?œ"ôž/Ó?ó™U¬"ì?º§—U"þ?§{1¢Úøï?í'CÈgôl?µ§G¹j?lgä•?'Ã\á'f?°@TȞÏ?´9ì̎¼Û?çD‰7T]®?Ð)…î…É?Âx`wA³‡?É2#ÌN‰?Àuz«lÕÁ?¾då÷"ö?êiÇT€5?©"ì0¼Ìª?¨FõLt?™@§~ÎUþ?ÀG&`£(?¥‰YT‹ñ±?èÓ)v&'?º§À';Çñ?˜Ԓhø½?"âÍò]?É° óÚF¢?º€t¢œÖAGN4FGL J1550.7+0528¿Á~»7'Ø@EˆÁÛCÀ9œÊ
Õ«™À;ç þ}I@—÷û#Í:@,џšd›?´VÏÅzž?Ç÷Øi8'å@þ‹;26@
èØqÊ?ð¿ß'ü—?Í¿äD£""dS¿ãä'Ë÷º·¿íju>ÆdS¿í4€Û\²ˆAGNfsrq3FGL J1550.5+05264C +05.64?ïK äÂ?Ž(L)˜7–?ŠïȪr<°?"{Ô
#‡~?'LVkèÎ?}v‰…`Ž?•=È?›Ç-"›"ª?¶Nªþ‰?uSèU+?˜'æë*1·?ó éG–g?íÅç
:Ár? GîÑæYi?¢QAhâ?˜-ÜQè¤?¡PNAÄþ?"ü­A'÷?ì²£¦bÕ¸?ŠL—á9B?§Š7Y'?'éþÀ¯Ð?­Ê§¿cí?<bÚ`¿?î ë‡øÝ?¢å–½ß-©?¡ãËÝ\¾§?›ç(ÿ¹ÅD?›4JÐ×Ë
?'b¢(â¶ê?ìRÝ*"A?µú>¦Ø<?¦š‰ÁzØ?©Ô‡±XµË?²)IkØ?¬nö…gdf?ë.,͂C+?®<ª?·Í>mS3'?¨szüš
?­'¶Héã:?œ°Eëb2Q?çk6ÈûI?¡[‰À=?¿9 C}"?…'yàXÕ?¶˜Ëñä?˜Wd!
AGN4FGL J1550.8-0822?ïzâýÄD@@ól½˜|cÀ:ÏR]šæÀ<i‡¿}@!I³	,N"?û¬Ÿ¶Lä?ÒûOyx?¾G¼,@¥¸?ñaI["¤@/—b1ÎY¿ïh4œ¿¾Ç?ã#Mâáâ¿àYÕÿ{u¿â˜TTëꟿÂð@uœå¿áÍâ½ÐAGNbllNVSS J155053-082247?ïѯ½?h<ÔÜ\(?9,Þiƒ?*Êô™¶?uêæ‰P'?ghXwý"?ï܏Éy?q†é6‡?@}IK›îõ?KwXùÈr?oÙ6óAa?nëBuô¸t?ï_ì(v†?Îó¼Oz?\õV¤Á†Ä?^Ú³À¥M?'<í"Ö?€ñŽo'?ïs#gÊP?mÕ¹[/|?QÍì|~ws?=˜ËҟŸ@?\В3‡?m؋-ÛY|?ï¡7"ŒÓ?xØyr4œ?J"'ñf·?A.ë=j)?†o£j…?x
¡&A?ëæn?ƒC"ÝÀ*?R²z{s'?]\Ûr ?†üMBþØ8?¶½Nÿb?î'‰€ê?"œ•ú?fàF"ð‡Ç?dP{"7*?¥pƒ¥ã?"s»Ž‹ôj?î}eù·š?ŠÉ ê^Ã?_ï‹=Wõ?X+²Ýv¶ë?§(mGÜ+?Šî¥Û3|`AGN4FGL J1550.8-1750?ïìp3Í@@;oyB=À:f<OšÀ<#PÐÒëË@üZ.Ì@¹cc}?Áꀘ@Ô?ˆ³xy¶
?Æúw•bÓ4@Šá^<K?ïÿ|ý¬"œ¿æ/N6ĸ+¿åÊWÂ^´Á¿äBÞ6œM¿ïlbäѦ?ã£æ#µèAGNbcuTXS 1548-177?ï^ŒÆU?–À2=G'?büÈz?by¿±*»?'ÎæYE(š?•C{p]?ï²Ê"Û'-?|
W¡Ax¯?XÕòt'Ç?_Üÿ(ü»?€2œ…íJ]?v¨qÿnÜ?îès&ÆÆ×?u.ÏM?y*¸êZã?yI§¦'y?œ¦ìñãæ"?Œ×6Pg?ïäæg?jDm#¹'‡?jPVnž†¥?R\'ˆ?‰r°ô"?e=ÿá?îz˜g??¡·n®ÃÔ)?w–'ÕÅ?qFàñN?¥dA¡tª-? œ‡–©þ€?ï-×µoIJ?•4M¦‹ð?jiüP¦"2?sÓH'#Ü?–÷ÉÎá<*?'	Êcxç?í¶ôš¥?›èfjÉö¤?ŠômgÆê‰?"¢Â¨ª°M?­á2¥è´?—ÑŠr–=?î|ú63æ?† ÿQtá?ƒg̟*Õ"?oýKt?£VivĶ?ƒ\Ö¹˜dAGN4FGL J1552.0+0850?ítJ®`6]@EӜZzÀ:E`Kš2FÀ<b«esø@Æ;óS?ÿƒ>Éijþ?À6+ágC?¿9òj@ƒaŽQ@	ZP1›®r¿êÒ×¾Bph?ïå
`¬B¿Ý™–ÿáL6¿à6çó™À0¿ãš¯ú./¿ê71Åté·AGNbll3FGL J1552.1+0852TXS 1549+089?ïô¶i?Fߞ÷r?<n^zPu©?3~r¦ý±È?P¬ûcŸŸá?ANÿ2ðüN?ïÔX á€?sh š˜0ß?Ký"©™@‰?UÈ?ºÏ ?rTAºyQê?n¶ônâkÜ?ïÄ㔏n?iÉÿ.àÇ?QÒ6eça?8¥c^lšz?y¨:KÌK?hÂ"ïU"E?ïÆJ/V¸?blðjÍœ?sö9§Éa£?RжXšŠ€?'"P'/;.?]7~y\'?ïê/·Êÿ?Z*•ä.'?PYG8 ?GC|(‡ð?Z¤jª#›?S¡Fñ/õg?ïq¤Ñ—H?Œç+ÑG¹[?b wƒj?jŸ
'½Mò?ŽòÃs¶Ó?‰"¤é°'—?ï£ó‰=ð•?rŽê$Ç?Zƒ©"R?W$+ÿl?ƒÀyúJ-?p4;# !?ï$¤Çlˆ?}W áóŒ?"½†då?kÈSÒv@4?•Œ¤d_?w'AËÿ'AGN4FGL J1553.3+0600¿íص]Ý	@Dù‰7KƨÀ;6Yì yÀ<"¬X¸þº@®qÔX²I?ý7÷¾?ÚWÌOðÙ?êPåË¡T@¹àF&Tþ@ËBhÛ5Æ?ÕÔ:ªJí?ï•÷¹	¡i?â+@š$¿ç²_ä@¿èÒGàê;¿ïú~¯"®AGNbllNVSS J155331+060143?;:qI?¤Ü¦Áµ?‹'|&²•k?Ž¡qùCW«?  ÝB¬F?ž™6ýã³?í¹×e	͒?¯à
qgA?¡Qö'¤úú?¦tò‹™M?£"Nî?›àaÕ.?î/‡•¶
?žÊ±d¡?‹ÞYÈî?‰0÷|ô~?¦ÁG…Ÿ?šð•1ˆ—?갂ªÐß½?¡Ê«B5?°ë8wq¤Ô?—˳r2Í]?¹²0½'Å?š¬³Ñ™´?ìž ¾€G¨?²¤ýø?¥È"{Òt²?££ãM‰Ÿ?°*èÍ8¡j?©Ldð`?êò‡Ø0'?Á2œ8ÊÈ?±äÓ[øb?¹<î¬n…?¶†íߝÞ?°Ãvœà
?ìµø6 è?§ÏU@¸Ò¦?—¶é|{"?'ßd© ?´b¼•ãz»?¥ $>¡ñð?æfƒ•~àc?³ê¨ø(½†?µeúj³µÌ?§ø¦ý&Ô"?˲ôt¶M?²nuÂр¤AGN4FGL J1553.5-3118¿ï—Îåù@12—9m	À9Z—ü
¨À;ÃxØXò
@aÖ©?ý'RÛo&ÿ?«M—@+œÄ?µxs'-Â@
žÏc€@S¾	e"i?ïõäRûO—¿Àßȧú"¿ÞÚ/H¥5¿Û˜™ÿÅój¿àÑâœ'¿á`‰ƒœAGNbll3FGL J1553.5-31181RXS J155333.4-311841?ïëü݃Ò?U™Ï·?>-h0ú??7‰#%üµ?`=u¸³0?RcÝz4?ïÓ"¹W³?w/Ê|Ÿ:©?P1Ÿä=›t?[¼;Î@ùó?rb;žc›A?rZrÍ]—?ï'Âl£?ƒwJ®‰É£?l
ÝØ°F?sªPü?ˆLé©&?€V'NÇÇS?ï~é{?x?tՔoÙļ?lcøI"¡ý?L‹ÁÕ¥öä?š#£ÊÕ8È?sjÖÃ)6?ïÙ´á7»?h@%)p??I¶:†—¥‡?DõùÌt4H?oݏúsÍý?eN›'¸%?ïmëH–z^?˜ðõüi?f$[È1k`?tŠ«ò¤?Žüَ»À?•å"Áçdª?ïN7ȐŸ?ŠÝ
'a©?qÅz"²'?v¹,Éòæ?'ÌÚhà¡è?‡2é¬ïqC?í»•€7üN?'
Ÿð‰s?€K1ý8?eÙF—õU?°í¿pÊ?=kˆs³TAGN4FGL J1553.6+1257?ÎÇû !@Fš½çXÀ8àPšLGÀ;ÎtqÁä;@ïSpÁ@_æ\ÀË7?¨¿!œž6?¹ÏòF.®@
'âûã:Í@÷['¢Ú`¿Ú"
P»Ú6¿ãÖGj!ÜÊ¿â÷škP°ò¿çèŠÞ?æË¿êOP ,¿ïê=@RUAGNfsrq3FGL J1553.5+1256PKS 1551+130?ïç.šÈÜ?ZžE
òÐ ?F	(ª‡¸r?<¡˜7-YÉ?cOЩæÅ?W±æXðJ@?ïÜ@QmŸ¯?pd.4'$?B|H^"&?Pӈ#·¬Š?o ¨Éç¯ò?m‹z43S?ï'-­ã(?'Ÿlm˜‡?rˆÛlqF?zâ¹ýIÕ?'u+•¢ñ‰?{3àQÞH?ïø§Ð$V]?2Øê%"Œ?!¸Ý)t³?9=½3â?Hò½LbÓ÷?1}Úl	Íæ?ïÇõnùÕ;?r_wƺ'?S;`¨0;?I.lÝSÑ?w@9ÂH®R?pþÈÀì?ïÍ=?2¿0ã?U…XªË?lã*¼×R?Š
a¥-îÈ?Œ£ˆ¨'s?ïIT¾"pÏ?J:¬f_a?}zZnËa«?Œ›£ñÍ?Ží£#^""?…kJYs?ïíö¡7^?Qo†êb5?4ÊÛ‹V?%$u±W-h?^໳g?PMÜî*}>AGN4FGL J1553.6-2422¿Û+
\q½T@6OÙÛ©¢À8²
RÎÙíÀ;Ëãktà @\ê«Úä¾@sÄóºw?§MìGŠ½?¯)PÂvm×@iÝcóÅ_@}ø¸¸îŸ¿»aX"Ì¿àڏbÞòi¿åL'jP¿ãGÉÃ-Ú¿è{ß@í±¿ä@Ï_~AGNfsrq3FGL J1553.3-2421PKS 1550-242?ïÖs´ØN?®½"Ö[Ñ?P	Æ·Þñ?ˆ=/+(Ý ?póÛN™»?¨pCz4?ïß¿_?ÅW?n¸ö¨()?CwræÇÎ?Pöƒûݼu?kbÄwãÛ?h™–#v\h?ïµ,cdÌ?tšÑÍqž7?Xõ•äpf÷?VƒÍÖI?,‹Wñ0j?s`Ë$1´Â?ïåê¶ÓÍX?JôÙW1´?EÖé`/?,Êvâ|Ýÿ?d­Ósî+ó?Hcf€Èè?ïæ]m!;?ZµžÄ¼%?BߘsÐd±?8ËnÇFw|?dê¬Ù'Ô#?W‡'C³­È?Õü4?'·ÐâJ?UÑ·ÓL?g=UXš!?"ö*——ÜŒ?aÙ&ÿó?ïnWˆÊ`Ù?…^0î҉?f"ïÔÍÂ?eÃÚ
Å?ŽÄâº:?ƒðƒ_Áé?ï»Ë?ô?kF‡ˆ?^…È8ãÖ:?Kø¾í?zxÿÃ^¬æ?gՓ̤SŸAGN4FGL J1554.4-1215?çÀ'ˆäs@>¨îÙ8À:­ÓÿÆõÀ<S'üžK°@!!šû™hò?ùÑ÷®ø¦?Ñ"ð½m?ۅlÜ!S@pŸ±@NoMjÁë¿ä3ÍêÙþ¿ï®3ïñ•?íé°"G'²¿±ìµàÍ	Þ¿âҊ¡"³¿åv_¢ýÆjAGNbcuGALEXASC J155432.61-121325.7?ï"t–!aq?‹Þ®+	¶?s#ȞÍ0?‡x¾"}?…[ȞVý?x´Éö®?ïY¯Ï?R©ãAB?vOÚÇ­òK?xTzã™j'?ŽlÜðù€?"¥^Epý?íúG›íSL?œév^}¥"?Œ™ùGµ?‹BSµÕR?©5A¡I?˜{Aàb:d?ëó>¾#3-?š–­œ'n?Šç_ë»	?uE-¢ÍºP?½	%*÷?š3½1A6?îæ©­ü?˜µþóô* ?…4ïø€AÊ?‡; ´ÍÉï?˜¡²Üzƒ™?'>ÐÜb'?î/›×•
?¨mxQÁ?Œå‡ñµì4?™JËsÔù?¥Ìà•léV?¢m²þ'?ë®w²Ç›"?©±x®ï@?•'ºŠ	R?'9~"†?½+"Æ_º?¦só4,½?çŒØM‰uµ?®ÊTôåIå?–çèÖÑü?? @+-?Îï¡ÅÚa­?®ÿ¿Ìç AGN4FGL J1554.9+2143¿Ë²Ý|6K/@H
uÍ·À:ºà¨KäÀ<'sϵq@ënºGäñ@Ât֐›?Ê<Kö"±†?ÑqP¥4@‡Š£\û@ó…mèÎ¿éòUóQ›Ô¿Þ¯ë¶pj¿Üž'¨'Y¿å×ï_ô²D¿æITrHù¿ïåXÿöoÞAGNbllTXS 1552+218?ïwjÕ-eá?É«;ùÇ?f;—ñNè?]—ŽQ9÷ÿ?Œ"ûÃS~?€>['¢$4?ïš^p×6;?~%:¹Åæ?aŠ­;a¨Û?ap­À)¿¯?…¸‰pm?y¿C˜?ï$xÏìß3?ˆÌÀ[¦ú?z#°r°?x1€ŠçÀ'?"è*Ÿì?"^ÐCô|a?îä3'ñò?u]Z?»Ó'?'Œ#ƒ¢•K?a"²å?š3{÷U1?qÈdԇ(˜?/q»7?˜}*òÉ|?xDi.­"?r?™3rg3?£¾ß䬒p?–vÜ͘F*?î–Ôn܂?¢ØyèÊu?yT1^ŸÛ?x
Ä9"sÖ?£h:¡È"l?¡ÇβƒŠ?î sp˜¢?™"]Á+?.gÜ*ð?‡—=¶ÔCã?¦vÄÞdüc?"îPƒ¼Ø?í	£ a<?'ùt-uðL?"ªtƒÔ?|œEøà	–?²ˆ?»«?V'þˆèAGN4FGL J1555.2-4149¿íÔf³U@"
?·¥ôÀ9eR1%;úÀ;rƒ]œ"@š–pÅ:@eÐÄ©Ý?ºB÷ ˆ`·?ÈÏÒ»¤0v@üÿý@öQ'S?ïß¹£ûk¿ãâÑñÏ»•¿ç†‹À)M¿ç|ŸÃF1¿ç:hŠ'¿¿ïüÇ0«™vAGNbcuPMN J1555-4150?î¼ԂΧ?ÂcЛ»?ƒ×Á¿rÝ?¤:}ïùã?ž'D‰½pž?¼	·ŸûÌ?îå¾5ZU?¨Øym !?twä
©™?x8uqWi?¤o5#°{?§[|"^>½?î±°°%f?'wÕ#³co?ƒŸ¹ë‰?'y†ß™·X? ¶{È:{?‹÷Í_!8?íàÒ!dB?†­qs?'V½þ0"¯?dʍ°ÁÏ?­].gôo?"™éó°?íXÎÙþtÌ?Ç;hƒD?v±û˛?¢Å¤°ì?±ܲŽ9?Âð#šuô?ì²m¯Ÿ¯!?ºÆwÐ?…Ú~]?'Ö4+e)?·±BÌÔ?¸åeÈï?íÎeñ¡mx?Ÿ'‰£Ùî±?"ú-–×?'µï2؀?©'#Ói«?˜wKÆ9ü?éR¼úƒ?£ØR¬"*ì? D¹ØÔB?…4³|ÚR?ƦхÄ$³?¢˜µ?`çAGN4FGL J1555.7+1111¿ïã¶"2Ò2@Eû~|âÀ6{Ãiv¼À:xßN¯|@üØ®,x¯?ø¨–<"?Ž¡öVÖGí?±cXÊÇd@¯b_p¨à@²‡ªƒÌ©?Ù͵à¢Á¿Íù2±-4¿Ö3=ú·k½¿ÐHÏÃL¿ÙQºÀ/Û¿Ù.šG>'óAGNBLL3FGL J1555.7+1111PG 1553+113?ïšøÝÝý]?'6§ó(Ë?lØpMÏÒ?ƒX >@,î?'Á"`Ý?‹.†ÁžÈ?î‰asôª?°æ¬ F+ê?L£²ý6Û?£Àú~[Ç?Ÿ-«a@?¢ýч´¤>?è!ò$?±ŽáR´…?§eÉ}ÝÉ?Ÿâ=ÆöN?ɞÅ+ÝmH?°HbÃâ?çû\`íÅZ?²ãW"ƒ³"?—3TºC=?'}¯·Ìã.?Í ¨è›ñ?²á¦jxÉß?ïBI©ÊÇÂ?®ÒãÊɯ?g
ô—¼~²?mìÚ-`?"Õ2ÿ‹Û?®¥6ᷗ;?ì7Öa‡?¶?À%Ÿt­"'?£®Ýwº­®?´7ëÙ^Sé?´iÞ7è«y?µ3Ǜ14°?éb•¶"f?°í)v~ì? _Íö˜6?™"‹
¼a?Æ]¸jÈ©Z?°Dރø'?ãÎù ‡÷?À"ªÍ§ê?ŸW™îí`?"Mûû'lð?Öl" ٔ[?À䍍
®ÉAGN4FGL J1557.5-7040¿ïáÈEî:ŸÀ*Odñ`¯À9¤Ãð…8ºÀ</)¹6íÓ@ąrp4ñ@ƪ#T˜ß?³îÅ`ß$?±7Ä<…lf?ýQ‰)ßÍ[@Ž88€¥?ïëÿ,›i}?Öwz?·%¿äV4ŸÄÖß¿Þ»#­Y¿ä5YžVí£¿ænC?ñCAGNbll3FGL J1557.4-7040PKS 1552-705?ïwùêÎPÂ?~Âð.î[?^Œ0¿)e?PÙAí¹Î?ŽAsÕÊ(V?|* )1!ï?î̇ô?¡‹]›¿ù?‡èžŒº?ˆxKp_Ç7?šˆÎº•?œ6rÊü&Ò?œÒâ?"Z͙
?'1éÕÆÄi?ÍŒf? ÷Û¿êøB?'ºl{?ìNÉ،ګ?'`¼³nÎ?©¶_{zD¡?‡ojt|¤w?°®|'-Ý?ˆ ê¤V¿ˆ?îØé!…ûq?ÿ=l¯ò?t¼êp
'‰?e³¤*îËb?Ÿ³¡*þŒ?ŽöÜí`¨þ?ìÕO£èc<?¸Ö5F××w?¡}ÁŠšp?«Štÿڋê?°–¢"÷f?±°£–Ê?íZõü¾N|?÷ñsO?»ÝÉðÚ?†›Ñú€†›?±pÔhŠs…?™ƒÿÿT3‰?çmÝԏ—k?§È¢±i¹?¿.}ýíè7? â(³
U…?±I®Ê®:? 7TDĸÔAGN4FGL J1557.9-0001¿ïƒ2–øvì@BÔÝÖàLÀ:®]Ywj›À<3nUH0ñ@¾x,a‡Ú@ŽÉ¹òÕu?ÑÆláTÄ(?Ê5öHÇ?õ.éÝ~˸@hØë>'¿äùn‡P¿äÏ© ø³…¿áNƒ†1ÝÉ¿ä­¡ŽZ¡6¿î´²ú"¯¿ðAGNfsrqPKS 1555+001?"»R?™]s8íî?ƒ©õ…l?' F0	ãÒ? `ruW4?"°ÏËlÀí?ï­Ít¬>&?ycñó?\I3cNjÜ?`¬`•îÆ?|r%'&?t#«›™·î?îàòŠ1ØÑ?·w÷pU?‡*›9JÝ?…›©uL?˜La#þ¯??‡üˆê.ci?îÛ³ž8Ëà?{;0ó´ãb?pu`…Íô
?Qšù•S þ? 6w‹?yÛ©¨E?íAX\Yê?¬.š7ÈE?Ó43Ó?…Ö'–&Z?³É(2N0å?©ÿÙ¦R<?ï‰j
?™Ç`œåä?lóˆóaª?v—3ö˜l?™0n˜öÙ?–4pŠÓ?ío–1@{? ¦.05?—çˆt_!?¼†#]6Ä?­")$N"l?˜Å^ÜhÒü?í$['Bªl?–·œö³ë?~K¥Þáù?i9ÃntêÈ?´û>¹ÉñÃ?•Í¶¶ooAGN4FGL J1557.9-1404¿ª"pmzâ@<Îü›ÇqCÀ;ä܎
ðÀ<¥³7ÐPæ@ë%ŠÔù@U—Ià?Ò)õ1oä"?èQ¤7'M@›ß°Õ @¥õ¢"?ïèçë6D`¿Ï¨ýz>µr¿ÆQˆöÄm¿éprž®"¿íTÝ!®¦q¿ïþÛrýœAGNfsrqPKS 1555-140?è"ä_ÕA?»{¯Ÿ{—?¾ø¼·"bù?°Ñœë ±î?¿ð N?³_Xý?çÉr$_°À?Ä)¹•k?ÇðãJ?ÁÙ
,¹Fˆ?³tŽª.ï?¤P=(÷?ëZ‡Ýkº?¦DB<J?³	ŒÙ(?ŸyÌZ(n?²"¿‹óH?šó¡UƒGÑ?åFûâä?¨R´rí?Γ­yFN?£{gŒM£?¸ ÆÑK'Ã? ?¢€"¦J?äþšµÖï™?Á~,'êŠ?É¡¿ÿp\?»ÓC£1¸?ÂcÕ)4#@?µ8 ]Ä\?ß\ŽF7X?Í!•;úº?Ø?¤@øª?ÍêjÂk ?Á$d²ËÞ?²çô¥Þë?ç•Æ'dàÄ?´<Àɵö?Â"à2–f?­•&íO…A?¿@¡¬sÍ?¥Ož•Æ™?Õ[ís'Ðø?°Û›ŒL¥?ÝeY	P?²=•kDn/?Ê}sÁûZ?±Žš$=}ãMIXED4FGL J1558.8+5625?íÓ Y.øï@Fá«\9¼ºÀ99¿×hÀ<J໗@Ÿy•în@iåŸ+©Ò?¬þ¿õ40?­$g_×ùH?ýFÈ •¡½@Úœ&g?ïÌÔÉ'¿äÒ`v¸C¿áÃq~óP¿Ý$O\^¦¿ãwomv% ¿ïÿòß0&¹AGNbll3FGL J1558.9+5625TXS 1557+565?ïíX§¥º©?ZĀ™½…?:ûî3/`?1‰ˆÀ–Þ?^µz­¾'?W»'»Q/?ïÌé,¡@?q˜pØ7í‹?M¶TG‰ùÇ?T®ã$I'Í?v<@âñå?lâŽÅsÔ?ï¹øÉ¢BW?uŠ{áþ-\?`«âם?qD·"?z­Òü[ę?jë‰Övý_?ïΈbëê?WD96H¹?fGêaž.?K$Ñ8Å!?k0'
ÏØ?N)YxñX?ïâëí¤]Ã?c´@.`?FæVøë|Ñ?>}k1¢N?gZ|Úº!?ag'Ž‡ÀE?ïsÍß
UÞ?Šùùt®OJ?^ð@/'?iªzÑþ?Iê@o?‡Ûh›õ¿_?ï‰îrRǒ?€þ¿©DÒ®?h€´Å•Þ?uvç5)g¸?‡d6C/•õ?{óUÞh"?iªéx?to†a·¸?|¬ûá	]?gJÎA®Vƒ?€
5•M?h¾Ã›ßè³AGN4FGL J1558.9-6432?áylÿÜÀ!F‹;26À8©1½nÀ;ÒêVJp@²X>…vÍ?ÿA9k[˜­?¤âb¶-¤?—Wºã&'?ñ²žÓ•=ê@פ"G ?ïíH"-§X¿Ù	ÿ}y'‰¿àS™Û¿ÞSCο஗WŸú¿×uq{î8AGNbll3FGL J1558.9-6432PMN J1558-6432?í3FV¯â?¦ëEz0éD?q_Úë"j:?ce5⮗?µOϜÇË?¦%/ò-{Ü?í7­S4ÛT?²S8Ázy½?c"våt?m´¥_/ÆX?µ©äT"Íý?²hÞ–}?íŋͩ¸?ž›}(݊X?ƒ	¯k?'­—iÉáK?®ãÀ¶íQ"?œb>Rdë?Áe
?'…úë@Ú?‰taÃí¿±?js&I± ?¡9›|#»<?}ÓÛ®ïƒ?éêí:Ök?¶üð®ûÁÝ?"š,¡s?zÃ^™Pd?Ç[J~?¶<T'"Û?é¯Ñ
ì?Ä©BYðØ?vÒK‡(?‰j|êo­?ÊÙãè¥Ï?ÄG½™S"½?ëÕíOy9þ?¥µÓ£5Á?‡­¤©È.æ?"OÛê´Ú·?¾Zàî6·?£÷2#"7´?ìÉ5'\«?šÅWYûkh?fhoR(?ƒ§³Å`8!?³¸T÷œ?•W´}輁AGN4FGL J1559.1+6736?å""èe7E@DcEŒÒ
úÀ:ö*rDÀ<á‰$@›½Ñb^?ý…‹ûKeY?ŝ^J82v?Â3Eèª;?ú®ç¸5f@M¥ÿX¿Ú(ç	D¿ê¡uÁ"I¬¿ÂA…±ZV¿ä mòKâ¿ÖV>{ë°¿âž8ÀúõAGNbcuNVSS J155856+673646?ïÌ6ZÁ'ä?hqvß?Jãæf6¾8?;h+/Þèª?vˆUԑÊë?fzý¨?ïÎÏÿ1N?q‰s7jZ?HǽUúË?Pó@—[d?ušízl?mŒªš¶5Å?ïeUªßðŸ?s£ë§?\êåPüÀ?Wo'»'á?'†œKV"Ö?©ƒ)s?ïº)d°â>?Zw¿Ï@I?U¯$æ×I"?;9ðn-n·?}"`ʊ›?Y£õò¾?ïnuâìZ?"ÏyÜW1Õ?dwËh/ª?WÁJúÛl
?DÁf$D?ƒÓA'?ït˜Düè?…ê6¾MÆ?Y½,}w?b™é"9y?¢MÛ¼q?ƒËŸºÀ¼»?î¿tmä?R±_t?dÉÎw?[|ªs"6?¢¼'5"…Š?Ž•ùõü{N?ï3ÝxIEw?z¨£tÿ#i?hZR®d.?Wy7夨ú?–y .é_?yƒ²ùNLuAGN4FGL J1559.8-2525¿åô(Ì@4'"àÞÓÀ:^ם
gbÀ<#¤¦©M@éш'›@r=Ÿ¿™?¾húÀP¿ˆ(ÎÓO?ÉÏa<0@|ža)'¿ã_¿"å­¿Åÿ{&<¿çL_ß¹Ž'¿æü¿ÔKK'àD¤¿ìSŸÍ:[AGNbcu3FGL J1559.8-2525NVSS J160005-252439?ï~PDˆg?õŸ'«ˆ?`UFÂRê?QŠ–êOÖ?Œf™'–Ÿt?}¢ÅÐvÕë?ïÑiô²¼M?r'MĘD?CÁn€Ù$?I'"Ør	©?tÒ×Äõ­_?q)ÓᅕÒ?ï<ô'üÒ­?ƒ£"²2hò?i˜Ž·Rd?aç5ñz?•.]ÎvÌä?')Ìý&5d?ïwï6u>?føα—}?T͐ˆK-?;@íTÝu?j€dYêÚ?f«^7JÉm?îžp{ñ›—?™Èî˜dë[?v1¹§©AJ?gèn=ö/È?£RÁ	sfí?—õ
§¥€@?ï{:ú/?‰ÄP3Šä?Tݒo"D"?`ÐMµÁ?Ž•Ã7¦?ˆO5Š_ò?îô@pÅ?˜†Ó׬»?~"¾¿tÞ?tDjì²›?ª®'Aα?–iLõ§?îh" ÄÏ0?"î㟍~¢?nú),y§?]ûÝ7˜'?§Ž="0	b?"j)¦®áCAGN4FGL J1559.9+2319?âžPøø­@G¹I¾ó(À9ßÛz¹×À<<¤:Œ@7'&«;@^ÁVw?³dŠn-…?q½
«Óò ?¾
~BÑ
õ@
æéI?ê§Tm@?Ý¥h"αS¿åŸÁ}ä1¿ä3aÁ»÷'¿×áËÌòŒz¿íÙ®'O"}AGNbll3FGL J1559.9+231987GB 155744.0+232525?ïêkPu?ZC9À?=ÿIz1_?4ƒ"Ÿ {"?b<«ûó‹:?V€§C«o?ïâ›âãÔ??mÐ^dRҘ?=ÿ]ƒiݎ?IÿQ!ËàX?i¤1q=å&?hèa<T?ï—Ö´4Ù?}vPeß]?XóÍÉÍ@?V&F—â?†ëÙKn?|ÇÓÍÌÃê?ïÍÞÖBJ?Vò'|ôƒ.?^þrJðö?Fދր\?qPø-â0?PÚËc?ïÔör@Aí?išëISÌ×?PcÎô&Ó]?D³·ÖÃÇ­?qkÓ"ÕTŸ?f|ì÷Ñé…?ï'~f§Ë?Šâq¼ÀA!?S/d9@	?^q=æÚÈ?‰=@lŸ,?‰4|'ÿyü?ï=…ëxÓ?ŒYl;n;?dP#æ©þ?f®ÞJ†µ‰?•Å>*`^?‹"mÊ%+?¿×h?rñL©"ò?sûÏ/]Z?b/Rn-ûQ?…ÄzY=?lØÅÞO!AGN4FGL J1600.0+8510?ëD7ÒK´+@>Z_¦XĽÀ:š""œÛÀ<Š4 ˜ü¼@tÊUú˜@bÑ6¿?µÞj(ÿS?¢¤Á¦?ë•ÏªÍž"@9"í];¿ÚÜÒČ¿ãÓșae¿áÚ¢þ)q¿ÞacÝu¿áŸÑâ5iÄ¿ìÔUøZQAGNbcu3FGL J1559.7+8512WN B1609.6+8517?ïßÜ?uP?W¾½(?Lˆ`tYTø?9BÚ_:q?iËŽIök?Sε~ï?ïÕvxœÕ?tˆ†È@Ö÷?Ll]0ÇwÈ?Võ¥¦
ß?q·8ÊÔ?p#ŠÞ'µ`?âñsÃ?sñIp™À?bк8éµ?b(ᢩ,?‡ÜX¹ˆ*?pñ3ím?ïo'¼BÍ?c¨Òæ"#?q C†ÛXƒ?P™RÂß©ï?€HZ6€?_Ðêiü:?ïÁÂàÿy?pV]V±I?_µõ#'Ø@?R²€v'P?wŽ![éa?iäZŌÔG?ï"±ü?ŠÊÿÛ&ˆ©?`§Ëå?l]ØhÛbq?ŠöÚ¨²°$?†íÍ/£?ï2
C_{;?'y8©&më?q}FU‡?q±•	Ï#?•|x?‰Œ?}"ζzޕ?ïì½£(?_žv"F&?…nYé{:?lK¢À?"k6ý«a?xø·L¸AGN4FGL J1600.3-5811?â:¤"}¾Àœ¾|§ñKÀ9²~'ÖV¹À;³lsÆ¡:@$-"$@©öùÇÛ?¹H'OÐø«?Åz‹vì›@
IˆÅ5ÿ–?ñ˿ɯ?ïýqz–Ÿ?á`·Ð¼E–¿är4ÐÂ$Ó¿á™«ßí;¿çO ~ûˆ¢¿é(ž[ÙAGNbll3FGL J1600.3-5810MRC 1556-580?á[VØ©ÏÈ?Åù´!Ô?§¯þÊp³?£õÕOjZï?ÚSRt¹\Ð?ÅIàS'NL?Êq´XÚª?Á:fè0DZ?ÅÂD;Kä
?¸ó	9@?ãóÛ³€²?»»çfÿ?çQóßYË?®
g6c÷ô?°sÛ~V–?é³5[ˆ?Ê~DmŒË?ª§{ô1?Õåjà@Ž?¡wóûéì?Ô´éži?¥ßÒ an?Õfy6!Ð	?¡ÓҘœL/?Þ?rgŒ½N?ávkÛßÿ?½«1ü?¸H@dâ.?Ú{âÖñ¶3?Ãy"m_Õ?³¿9TI(I?°í­÷Wa|?ÈÃÕ«ÔÁ?â-ô§S¹?çWTðhç?ĵ4³C—b?âX¤Ý¡?³­â䬷?»X¡ÊÉ?¨'¤àyÆÎ?ÔyªB€¥y?°)…å{¨?ÂÒ8^7»%?ŸÔ	f=?Ü
®ã5x?²YâîæìÍ?ڐÙ"ìö?°Ò'χ˜MIXED4FGL J1602.0-0641¿èð˜‰NGâ@@lÚãæÄÆÀ:ÃÌ­ÃJÀ<J¶¶^Ì@\ÕOÓ'@p̆Uï÷?Ïz4y"P\?Ò_Û\Ý{œ@×z€ÎÇ?ñ"icñÁú?ê¬aBD?íAd®L¯¿á-¹v®³¿âñ.«äö¿é–}_Ò"¢¿ïþ¢NZAGNbcuNVSS J160146-064256?ì»p{¾?°ª}·MÐ?¥ZOÍ_Ô-?¨‡ø'0ªõ?®ôé//Ͷ?¢ÁÉÕÊÂô?é}{64Íñ?Ã>>öW?ÀË
3^#?¿³Rþ)¼?²~éU43?­?,3[ƒ?í?³˜¸? )¤å¹>? [~µJv²?"õz¸0r?«©G¿4ÈZ?—|Z&c­T?áa,T5¦?¨b0ÝԘ?͋ߘg¦"?§E¬Qjv?ÌïoÁÁ	? ßë~?è™F0ª$?¹ªÇ1ò?ºB
¼qŠÝ?´õe4ߜ
?ÀyáãŠS?°L¹þ$Cè?ãi	ŠS'´?ÌÀU@àV(?Ќ©.ï?Ê4N}ÞÊs?ÁB‡¢SÚü?µ>Ì80?êŒsˆZNw?ªÎ÷:Û,?°'tˆÔU?¡FÌD?»šÑI€žî?¢Ÿà¦5˜Å?ԓK`?t¤?ªL€-¯2*?ÓÙ1	7a?³¦£¾Ä?Ø[Ûn·Sû?°4
Æv£IMIXED4FGL J1602.1+3324¿îÌþy×Ý@HZõÊÀ:ŽFipÜâÀ<¨´ú¬@×	µ5l@k¤"ÈŸA?Á8ø²<(?¾â_&ù?û‹­b¤:@~ôþð
•?ï¥^^Z(k¿¢ÃÂbÀ¿å¯Ö(ôì¿ábòsO'õ¿çÌÀ7"D¿ïõµ>:Î2AGNbcuOS 300?ïÉÝe	?l%Dýœã¥?W}²ãÕm?OÞàc'à?u˜JñB(?hofAä5?ï'ðÈ‹&?"]XmxØ?krêXýàÕ?oû¹î§~¼?ˆg;ob|?|½j†ìûº?ïyˆEo‡?v¥½<ô?fTbÇç0	?`ւ
5Rè?ŒÕç}¨!?sZûûkÍ*?î¿ä¯A¡‹?y㣋z ?•®Š{öD?r6^GqKL?'ë»'wBU?p+Ҝ:¢Ú?ï~ó§›Ô¡?LKfg‰m?rŠÛ7_?nD»]ôð?†ý¨4?vúѓ‹"?î«^hž­ˆ?œËRŸKÅ?~­ Ü^Þ-?ƒ¡øDî??¡teYUn¸?—ÚJ¹·œ?îî¸HAžl?†ï"œ
ªV?x¹ìïXÈ+?rp`¥†0·?›ú{º>2s?'¥Ò©"ð?ì¢å~ä%?"û´?,þ ?«©Á.­?­ˆ™)!Û?ª5±ãstš?‰S7(ÊÊAGN4FGL J1602.2+3051?í?^ÓR«|@H5Þ½çÀ;¹†žëÀ<¼}ÄY@×kÖïí@mç˜ã?ÄÅd"¿H¿¢ã	'¾>r?ý/|&ìþÆ?ïîýy=¿æÊ?d‡¿á5tV2¿ã0‰4LJé¿ÔZe]Që¿ðAGNbllRGB J1602+308?ïÂhºuÿƒ?z?U±kôK'?M
;!=|¦?y_G܋"]?w§¦&9?ïªf@W´?}WA'Žœ?WÃ@`Tm?ZúR=¥Ø
?'n¦®¼?yG²ûüy?ï>
aOG³?€ºZ´uuÊ?j¾Ÿ³_¤?aœóäÉ?"æâ#€u¢?Ì[ ¼˜?ï˜||ìÿa?fÅmcEC?h'ÝÕÓC?QÝv<ñ¸?ƒ¼ZÚ@Ú?cv¿P·?ï˜X´L"m?€u ÀÎ<"?g‡†aÐtã?a›ÖB;î©?"ñ`‰é\?{‡£Ó§X?ï˜ê$Õ?š+¸cµç@?c‹â²Ø?kŠ, à ?šŽ0—½ðh?™m•Åÿ?îŽ}™™U?'Ah¥çÍÞ?ul†™•E?lø€¾"9?¤ubU%DŠ?#f牟M?î½4Yàn?ƒ‰TA뛼?îQbæW¢?p±8ܒU?ŸbLkÞa?¾³0Û¢AGN4FGL J1602.9-1928?ÙújÞßãš@8C(ÃnÀ:5s"u"*À<([{PÙ6@<MŠ!…@\ޅ[ôó?Òõ»ƒyG?µp$À©¨Û?ò¢êÊ
Ö@ŒrêƒA¿²#½tj5(¿ã6 M}aU¿á4DZ°è¿Ú"UÅYeø¿æTÞÿQš¿éUõÀa¦AGNbcu3FGL J1602.8-1924PMN J1602-1929?ïßIû\éK?[·–'z¬Ê?Bñµ'Ö,v?1¬~×ê¨^?kù—'ó½¾?Xó6qÂÂ2?ïÚ­éê*?pYìþW?DÔÿÕñl?P$š	‹?pkžû«w?jˆ°,Ëí?ﳛEô´{?pù=5›?Sõ¾É†t?@B¿qX?€šûÏÆ\?p(]i'?ï<Ðàz $?g $åFÿ	?jêÍ+ªóE?Bئæ•þ›?•ŠQÍß?fb3ØõÒ?ï¾@ˆí`&?p®T¢}È ?R©€_Àh¾?C~@õy÷?|5[gÀê¨?nÎw­ò¨:?j	¼?†õÁ9?[jó<šßn?d¢õ:
²?‹%Ǫ…?"%E?'?ïYQG›J?"µ‰/X?bÍ<é}M,?]èsuóî?'|/fÐ«?ƒElЁn?íù\xY‹•?"ÎaPí£?ÚmðV"W?`¢:êš»?¬nêº
·Æ?ƒ=•(ÇýŒAGN4FGL J1603.5-7112¿ïßåä~wÞÀ+đ)ˆ†À:¼ÿc"HÀ<3`:Ó:¥@*Ÿ"ƒªð@û¯S?B5?ËÉB	9å?¹¾'ø?Â8?ñkŠ'•™Z@¯ËE¥Q?ïü	 ?
¿èâÒþ?5 ¿çE^í{Ä¿à–±RF¿êtjÀ¾ ¸¿ïþ°à<4AGNbcuPMN J1605-7112?îã§qôd?"+E`ÙÊç?j×ߜ%™¦?`¢MûD? 
䏫?"‹?£Sä?ïX¨k?žð»Õ³Å"?u1olRV?v™1àd?˜ðÃßÙ½ù?œµ'"Ë¿®?îØõŒßvó?•^çæŒ?|–ÆÂ"û?{Å5Ú"é?»œ¸WÖÉ?‹jî?ÌZ?í!pÀ²b=?‰gàVDïÄ?ŠQNM×)?en¦4]Xä?³²Ñí
®?ˆ‹ŒÒ?큺ÿ‰§M?£ñìÍæV?}r½ðºŠ?q~Oíý>È?² Ù¬"-?¢1´Õu—ü?íç­ìÀe¿?³TËEy‹ü?ŠÓ–‡ÄĐ?–S*È¡1"?ªÐ;'äYí?°ó´ÏŠTH?í¹R:h ?œÈt2ãD?‰Š
€B¢À?‡_ë¾x¢Þ?®\›G?—¡!lD}?ç÷ù"Cy°?¢²ÃVx|? ®uEgÃR?†F(Úôë•?Ëô|œ¼Am?¢]a0ÑÁðAGN4FGL J1603.8+1104¿á+t‹JÔî@Eü'œýÒÀ:¤Z7ƒúÌÀ<Kü²m¥ö@ñ< e'@ð?)á{?Áà;êf政U³·µµðB?™¥Zˆ.@‡hÆ=­¿ïž5_³Cå?ï´øÐ`ֿ暉ÿÖ%¿á%ÀN9H÷¿Ù°L£òý¿èò5ÂY¬DAGNbll3FGL J1603.7+1106MG1 J160340+1106?ï͗á;Le?eçtyì®~?Qùît6?@9?³!!??tµ"§™"?c´͕ØA?ïÛ½ˆŒ+?nçKkŸÉ|?C7Ðŕ?KÕp _‰ñ?otƒ3 qG?iڌ3Å¡U?ïl2XËPÔ?}¯ücf¢c?a² le½¢?PèEs¢h?CpҁëÉ?|9²šÐ%?ïŒpÀ²b?d-ØíJÓY?c3Ì»ýî?HjlWY"¯?ˆ.°ªrÓß?c ƒ‰©?ïŸDÌ

?z"æõí(?b–urQçã?VjeªKéô?ƒ‰`qîÒ?w±þ¢­H‰?¦{n$?Š—|§Ôƒ?S™œk×y¯?_O¡¼rsz?‰ê"œ!Ï?ˆÒ]쀂ƒ?î¼@D'?"9±9?pέ¨mL?jfO
L?¢")!kÈl?‹ªŽ—.›¤?îŊïîÌ?áˆƒå,á?yœÚŠ³IY?fèZÑо? sµ°*ɐ?€ž¶q2ºAGN4FGL J1603.8+5009¿ïî0wõ"@Gz·ÃPLIÀ: ÌìÀ<§P;¶N@ ,¸¢v³?ûØ	@ñaØ?Âø'6H¼\?Æ1‰Û@ƒÛÂ3?üúWŒ®ÏŒ?鸊à刺Ð8Éà‰B4¿ÅPäÉî¡¿Ûü'œýÒ(¿âK"é\P¿à¿p\‰nAGNbllSDSS J160339.49+500955.5?ïƒíÆu"t?‡±d2üÎë?j)ª>-×?d‹¹=@*Ò?ˆz#é†oZ?"½¤>Lç›?îÞFVüf?•™ŸòÐÌÊ?…Št<Ü·ù?"÷ÁrD£Æ?™qûM?‹"ø6'Ôù?îúIú
çc?'Æ»0…=s?pÖÒ&)g´?r\Lnh¶?œ<ËÎ¥?';ÂlÚEr?컥hëâù?ˆàÑWC'?¡M;ða †?{<àÎéßç?±|6¾¸Iù?"	»ÄR‡?ïDŠÙß*?Œßöj¡?{{³;–ƒ	?q£¢nðÇ«?¸ñÞô?ˆB
¹îâ?ìä«osÅ
?°áœ$©Ò?š†.Â[ã?œð2Y_?²9ÓË›?¨=u<?îE#â{$?"lpûò~?'
…6.ç?'P¹ŒAW?§*mÝk:?™ä¤} t?è@Qò;_?¡(ý€Bj?±~µ›£w"?'K¶©Š®?Æ?]ixв?ŸHqD!(AGN4FGL J1603.8-4903?åK,ñr@›†»ÒªÀ7¶Í׎ǮÀ:¹oó­â&@ 4ÞÁÁÖÐ?þ'ü\'?£Ê`0žj?¯Ab\&ؘ@ŸÆ¤"Ÿ_@ô<ö*"(?ï±ÃŸ|Ý¿ãC´VÝ\¿áŸÆ¿l'ú¿ÚÜéåâGˆ¿à…_L–²¿ßt¤9/ÌAGNbll3FGL J1603.9-4903PMN J1603-4904?ïƒ!ë멏?…ӝ֨k?Iˆã‰©?B'*
ND?žö˄ëe?…N"S1êÚ?îù±¢$½?¥YþĀH?Nفnês?hœs'rz`?ŸÒÿ®ÛÑ÷?¤ŸçD$û–?è,!ìn¡?±Q…¹gë!?–Ú~åX÷Í?"ö-%-?Ìt(s,Â?°Ž£@hN>?ïI¸ÏaI?z«Îói(î?D''U&r?0RdHJ?–7÷啠°?zYa­I"?î…x8哇?¡[hïHEì?ZXgQs<D?U",(ëš7?¦Õ¹:¶Äª?¡ÖÍ7Èó?í<úÑÓ?¹ð$3É®?[½¦Ç5þ?rzãÚª?µ©6ªíò?¸ÍÔ³Ìß?祳nèý?±äÔ×Ü?'p"¸owÑ?d§è_?ÏÍó	ð?±Oœébã-?îRö>'"?"•Ó'bš?XƞBŸYœ?G±f~­.î?ª
g%Ø&?"m Œ`£AGN4FGL J1604.5-4441¿árÓÚ¡æ@­§m˜À8ŸïŽ˜´—À;Žh
/"@_«Jqg@Ez]"?­NÀàãã?µÔšaÂÛ@©ŸâÚU@ÿ]®1S?ïéÌ¢Zˆb¿Ûf&ºÿÅÈ¿æ'f pbê¿âééþ‹á ¿ì,Þ_Ç;¿Ó5nA&:ýAGNbll3FGL J1604.4-4442PMN J1604-4441?îƦ¯¤i?žÅõ>Ç@:?jÞTkµƒL?…©SÒ¹@–?¡ç¯Âžø3?œº£`Šé?ï6éœCöƒ?šaÜ1œ?Q*"Žž¬'?f¬ÁžD?˜$.kIæ?œ˜Äƒ*?ë:ù ÃQ?«bóO¤uC?£ûÍVº•Ë?›6ME¸Xè?¼*P²0O?§_"ÐØÌÀ?ï)^Ñ¥,?{ú€9;'?\ÔÓñ'ó?DAT¤rôp?š†ê)#ò?{;Ec¼/?í=©ï°°?ªS~½Ä?sP Ÿ¦Ý¨?hՃOŒL'?´Ý¦vOQG?©©~V+·'?î) =ô=?®©ܦqŠ?\Ú}¼E?nbÛy†QZ?¬‡(9[˜?®IdˆKÛ¤?êF:õ§êô?­.GñC??¥pFÐN+?›ìœŸ(;î?Á¢8ÐY¨?©zŪ)ñ?íe?ìnn?™ÎñN¾'c?xöY,{çã?fe±æõö?³F›8Ý?˜ð0ÇK˜*AGN4FGL J1604.6+5714?îŒÁøï{µ@F^4\þޘÀ8¤§.­'uÀ<Õº²@±ÔÎÎÛ@ɐ¢zì? u ŠÜ_?³……žÙt@²¯CO
)@7cI¿×Qaz>¿á¤€-ŒÖ¿æ|fîK¢–¿ä/¥²óˆ¿í•ao0º¿ïÿ "_õAGNfsrq3FGL J1604.6+5714GB6 J1604+5714?ïÌ`yU4?p1¶@üB?hùàfgª?_Ù_L¬¯?j¦I~qž?güAI?ïVu¾¯8ù?–±å¹Úa?xZÉ£mE?‡),ك½°?Ž5+‹%?*"ý×?îè>ŽøÎ?š
=Ö¨­?}:ñ_Ÿ¤?ƒÃÀÍý±Â?›©s±qŠX?—ø1ˆì?ïÀCkSyé?aÌû2V—?s¾®† M?\Äèt—…?h@o`ŽN?Mr§[Å{l?ï©â¦öñ?€'Ðn5Fm?oÂïC'D¡?enk*3òÙ?{-4ù×Pð?z½çiùž]?î胮î?´?Èðï?ŽœXŸäg?¥
Þ¼˜µ?§Êa¿`ô$?­rë@;•"?î•{É ë? XU9iï?~þ˜F¿IZ?…!8LD¼?¢È|çúS,?žKowٖº?ï_ÏÛ
ñõ?Ÿð¿Pþl?ŠM¤`Ž?}''Š
Qy?{÷çø‹8K?h»ÆjâçAGN4FGL J1604.7+1734?ïĀü¥éš@FICä/À;(2Æü©3À<£Ø涂Þ@h˜ð§H?ý¨PKqîZ?ÖxŽ·«?ÓÈxª5É@ÖV%¦'¶@üçõG?Z¿ïþ²Þ=°?ïÿ
×ÊVÑ¿Ú%¬!†x¿Ö<« —¿ì¦>Ê.¿ï÷Ÿ¾÷¢AGNbllNVSS J160436+173324?ïS"?d?ŒplŠôë?yJa%öeù?rl¢$ã{C?Ž"jh{)ò?…â–§e£ã?ï"Ìô?‹oGó±£?p£3õ§?x!.X?ø?†Ž¢"\ÔË?ºj="i?íÁþ¹?7Š?Ÿ^é:¿ö?'1çO6??Š#oÝ
?«G á-J?›Ž"'T½?î4Y›I??" Œôaê•?˜Ý½'Ä®³?y©ßªÒ~v?¢=ۛ±FÀ?|Q™á½F?îI"H¡Ú?˜œ7õ?ŽR.CZ)?ƒ0Ü÷?ží¿Ú¢­§?"C‡¶–?î†Ç—%B|?£GEeä?†:çyϹ?ŽVSxìލ?¢·ØçJ?œh^pö"·?ì‰ÜK+2Å?¦Ì䲍) ?•—Ä%?‹Ó¼Ír±p?¶KXÝ='›?¤Ý²UÛ²K?ì^ YQU?›g0b^Ê?¡+y«À?Âž½É8i?´yFl§ÇO?•a÷_Ö%ýAGN4FGL J1604.9-3414¿ïðÙB7CI@*Û=ŽcÀ;D@\çbÀ<}Rkî@!…çïf?ü-Yvɋ?ØÔ Ö¤¼ã?¼'	AóŠ?ì"D¶v$@½_&V+?ÁóAÁ‰?ïÿ§¬_o¿Þ'{%ì¿Ø~¢u¿Ó$¹½üOq¿æ?,î‡ÞAGNbcu1RXS J160452.5-341407?n"{?¶?Ìîë?V"Éא§X?in'ƒlJp?¤âÌFÍ?µŠ—ؤF?îõûVšbå?«øc‡'Ç?ažm¬³¬?n¹LæÛ:?ŸÔ:.˜ý?«'G¯z?î‹î<Öl€?–ÁjIÔ?f`v:t¡?oÁ)%tK?¥ÛÐPø±?–bdL?îâr‹Lã?çj¨'z?^oÆ£K?H'ŒÇ2? èÔ³¼?~¿ˆR1â?îÍO\<?ªÏ-¦¬ ?c¿™¼QÇ?d'žÜLè(?­Â±PP—¡?ªO›å{–?íë!í̲Ý?¸èSQÓà§?n»Á—NŽ?ƒÌ†¹"¢?¯lUkPâÅ?·Áb@<??ìôP'x?¥n-'ÜÒY?rÇß
ÕHL?v²êf¦SB?·1ý‰—¿?¥æ}(,?ìî2llÕ?šP؅sº?gõ'/~þ¥?bÁõp…m?·ÎÆRÕé?šûçˆ#AGN4FGL J1605.1-1140¿Çûøߋ}@=½ƒƒ­ŸÀ:U%t9ŽÀ<,=CWm¥@ 
ä‡(¨Á?þ'Ï…ä°ï?Ç7y©d<ë?È£}É@-gAW¹$?ýîGSP´ù¿ì!"Þ™¨Þ¿¤öw@(d"¿ÏDYKK¿â:¹ÚÁ6¿ÞCùÿàË\¿ïÿy\ã/æAGNbcuTXS 1602-115?ï 'ô2?‰ë&=Ò) ?s¾v(>x?hÀ×°–è?—8ž2Z?‡<±_~­¿?ïHR§ö1S?3r^?x3&ê@ÎA?yS™Ñi?èáLØî?‡Ì¸Gx?î½D9üâ%?'
DôÉ›?''€`Ü8y?€Ÿ:¯Ë?ŸC¸ŽÖ5?ŒC;ÍL?ë£ÏŸSܐ?ŒŽT,½"?–tª'^h ?tvVµ²O?½DX_³\?‰¾Ýñ™R$?îÖ¬Ÿ…Â?¸-0úC´?ˆ<Eâ"õ?Û‹ÍÖq?¨Óƒ¹ø"«?™Æ_½ƒBe?íÝ
´'Ô?©ïzªHÆ÷?'áÛãÒ3$?˜›¶è$/?¨¾f˙¤Š?¡z)‡zíŽ?í4ýþj?¢| Mÿ?'_v"¬ý˜?Šú€Þ8Q?±ÃºPœ›D?Ÿùô¹'?æ`¸Œ?¡«¾š' ?¥#:`±Ã?Œ
u°ò€Ú?ЛŒ†iCÄ? PlêdoAGN4FGL J1605.5+5423¿í@¨¬‡@FƬ![š[À;;¡…÷%À<ém ‹]@ ˆ"Té'T?ú²ÜÌQ$?ËÛTyÿËR?ÇڇËeï?ýšR[íf @ò<˜Œ©F¿ïÿž`¨·D?ïß½4©Tø¿Á0Q"Ñ¿Ó^¢!Ód¿Ý.¿»Â8t¿éÃf½Ë¨AGNbllRBS 1555?ïÚã™7t?ZmA¨h(?Liäõ5ä?;÷µ·K³¨?n"	ԅú?W
@øý#?ïÌ*îk- ?u×ç	EmW?P°gû2¯?VW;È""?u¾nÙ[4\?q‡FÚ©µ?ïm´œ\ö?|çç
¹u?d	ÐÃçGæ?`Ó^—Q7?d«ja?{!ÆsÌ;g?ïNÅL.?lËÆmQ?uXW2ìÃ?VëñºFÕ(?ég?ÝÄ?hôE!Rr?ï½I&‹Ï?l9'Û¤šk?[;¯}¼P?KÈ(º§m?zŒ€Öýñ¿?i\wH
®£?ïjuˆS‡M?Þ¼ºçX?bêÚç[05?l?ó}îÝ?S󙫒^?Žtô¸h?îÿ´vrU»?ˆ‰9oÍ?lwÌx¿³w?cIbµ"ï,?œzw£!C!?†'qÁ÷º?îf ý•[`?‡X§JJ?'g;D™øè?nxM
¡?¥!Qþ2G?…F÷ݲþ9AGN4FGL J1605.8+7208?åno87 @Bõ¢ß"xîÀ;â©,´"ñÀ=2OŠÎ¢@!LçÂFŒ?öX¡fítã?×
£|ÇPâ?ÕÁ—Å.ô?ö
e´¿@_°
tM/?ïü¬ž"¿Ñì"xK¿î"'r4Ñ?ä𒤲ÒP¿åÖ<b0÷š¿ÁÕ;ƪžÐAGNbcuRX J1605.4+7208?î7Àì`€?¶£9O´?›`~Ñß^´?µ	DºSªJ?§o2L_R?¡Ä`>DŽn?ï¿L—Äh‹?z‰>ºö?ž?TÐÕìb«?`EÆîs…?{%~ƒ*yÌ?t§9æ»ÁN?íì"ðü? )I2J–?‡‡š
$=™?Šœe%ô†O?«TÚ}—Ü?-B(Oœ¤?盧»PE	?nu'
g6?f5Ó…œ‹?[¦K(©^·?EœYÎæ ?jPv¢5)ò?ØJ?¬Ïe}d-?Ž5ëLÔ>è?§ˆðc†¶^? J7¦r`"? 6"̨?ïM¯añ¦e?"¤6ÔÉ?eø˜ö*›?t/"´þx?"‹¤•¡? øÂÔï?íF»ÌÛvš?¢Ùt³­­R?ˆƒVž¶ÿ?Šæ}Dp¿¨?²¹¿ÏšNÏ?¡º'äS/?îë¦<üEò?'˜±»o?€¤æàd{?'Gtÿ z…?šåìÛv?‹!Wg'AGN4FGL J1606.2+1346?¯¾ÓdìhÉ@Eac^t)žÀ;]™J¿@óÀ<¥äŸQi@"j‰¶¢"?ûG'Æ}¥?Íkè.R#?©ZÞB ?ß³ 9†^@ÌR(–Í¿ïíû@R«t?ïûA
r¿ÛÙÒ#£É?¬öoÞ_Fb¿é2ŸÅ,Å[?нw¤ý%AGNbllMG1 J160619+1345?ïÔ7D‹?pp!ìßö?D‰
:…q?7j£RDY?sS\ÂzmÂ?nƒßé¢*?ïׄ*GQ?rHß#[?D …òŒê?Lù"sgX&?q©ï9¬Þ?o(.3ÿ?ïYîÇð€?'>ð¤0?c#ž|?´&?dB:þÔ¿ß?']ʹá³p?42ÑR\]?ïQåFÚô?u×MSÚ·?j6]I.4­?R»¦ÿÇ?'|‹y—ÜÛ?tDÛõ?wóN
?€…Y°õO©?Y‰«¸É–R?TÙXf†?… 쁉ò?~Wáì®9p?ïxI½¹3"?‹w°ùx£?Yë"ý Ê#?c¢ž¾X((?Ž°,"àº?‰<tØù?îÒ"ßJu<?·À‡U[?o'-fÌ?n;¾¹L´? å¯9òr¬?~žo
Î?îה&8?'/P¾3ÿ?"-{(b?pªTœÎN?ª>AïËè?'çq*ôýAGN4FGL J1606.3+5629?æ|vh‰y@Fbb#ᆘÀ;&,ºs.À<Îò`Û+@!"5Á­ßÍ?ûvmÊÞ¶?Æҙ•gÛ±?²;-}'¦?ếBŠ¿@}ã¾V¿ï¯IÏVêÈ?ïìá?J˜«¿à‡Ëp¬:†¿ÝɨÀ~	ñ¿Ã<òϕÔé¿ÞÌDý
,TAGNbll3FGL J1606.1+5630RBS 1558?ï×"aåßT?h•÷‰s
¬?<ºë"Äb?+9ù4zÏV?r­ƒw–~û?h['?ïß¡»š<?lÿ‹%»¦??ý+:{?F
+;1?l^٠7N
?i3	ºº`Ä?ï~·	Zág?uP~†çdü?V(¸o˜uJ??KsôJ3³?&ªÊՍ?tÂãŠ>Šè?z¢®R?a9ª@'ݼ?TËúDQd?@	j¬<·8?{ÿ°5"²Ä?`ìÚÇÖÕ¥?ïµùb=H?rԑ]ÿ]?MÒ9ã‡Üï?AmóĚ³Ê?€¤ƒÒ7èË?qîfPõ"?ïš~ZgÄN?‡a[4Ç?P´Fˆ?ZÖrÈád?‡Iè"ÍÕl?…¸£}¦§}?ï¬Ôù…×?‡qº}Jö¢?a¯m¥Ñ´‰?cTÄ«/·?"w°`''?…ö¶èûOÄ?ïAm#ìª?|)
ø^ž?hêÑª	ã?[@š¯ƒ7Æ?"µÝex?|°£+'ÈßAGN4FGL J1606.5+2717?ä…Ö£æ#¶@Gs¹8›RÀ:"¾³.–À<iÉØü…ø@
ÿ¸\}@¥Áƍ?¿)âýeÇ¿´{ç¾%ü$?ô05½Q.Ç@ÔL\$8¿Ô< A¿¿ç×ä'‹¿æ"[t›¿ã"8^kEH¿ç0=µm5¿å9̪hAGNfsrqB2 1604+27?ïĈgåd?g«DmÁo?D5",Ž?:ll"£?{~•Ÿ¾Ã?bXÝP©?ïÑåEÈÞ?rYG§Û?I'Fã™Ý?RÌë;†îŽ?sÝ`'½'?mî¾fÜ?ïl2ë\&i?"ø¦çz?aèóþк?b¥*:õÌ?<"<²š?"¢å*;?ï̬¨·f+?W.,&Ö?^|ó#?Eƒ-Ï¢'N?r
nÍÎä"?ROY:I!?&HƒýP?'Š%ûj®š?TÏÎâä*?N}¼îr§<?|¼g҇®Ù?'aÿ¾*Œ_?ïJâµû-?ž—‡uɔ?aù\åk¥?sI??"'Èz`Kù?E…0±?îÇk R‡?''BqÆj(?r §'?n õE+c?¡IyÞà˜?¿¢-ý6?ïX]¦Æ /?y.j¶ú?yæ¼g‹À?iJ}XñŠÔ?Œõ"â½´]?stòÿÊÒAGN4FGL J1606.6+1324?Ü>PJù¬@EB¹¡vÝ­À:â°"rÐÀ<OŠë€í@+^a_@'@ô	¢@1H?Ï,—Õõ?Ã,éØvN;?ò œÃÆ@RÐL^'~?í¥"à¿ÙSº|¾§¿æ¹þúFƒ¿âBH§µç¿ê$«°óR¿ïÿI¤ë‡AGNbcuNVSS J160654+131934?ï8ñöIjO?…º 9q?u}àámÌï?g‰Qõ®~ì?"'I¦Žè?'!裑ò?ïp¦ÿ'MÎ?ƒ>rX¶Ú?mÉk;àÈW?mt†´jxj?Œcå\ڄB?}ɱX·Û?ï->þ~±È?"‰©Èù÷?{0mc	?|ßä̏?"tÚ_–ðE?y{ û׶?î"dzïlp?ykͯô˜?‰èE×®/Ü?e>Îê"?¡9sFÒ*?uU™üt<?íYƒûˆÞ?¢·	0Ê0?ƒ¸f `í?…%°áWá?±òzÑe? ",VÑò?îuÆk$? Cýšoä\?Ù$©2?'y+¨ùø?¤¨zòŠW¥?›rÌ8Bà§?î  ¡"ê?"¶àÄ~ß)?ŠâҚ,–«?'ñ è'§%?§EJކļ?ùª‡oÎÚ?ë÷ó—oH?"ñÏnE`?ž¤ñª‰?ƒ>"•'?¸—'¬ã|?'˜+È
AGN4FGL J1606.9+5919¿î¯Û5¬pr@EÙßeUÅÀ;X)º
­hÀ=qÞ@‡qÎÏ[?üÔ¾¹
Ó'?Ò+ÖÝò¹ñ?̚Ž…ia?ò‹ºc=¼ú@
^<™8u½?ÙcqT2U¿íR-ÿ틉¿³:è‰@Ü¿ÝÊë€ìúj¿é",<žìÀ¿Î{ÅHIúAGNbll1RXS J160709.7+592115?ïæÕ¿2?cªò3›^?CÀ˜·Z%?8#ªÂ%Ê?diPÞ5F0?b£•KF?ïÎÎá"È
?rŽËKΤ?Gñ+ñ׈µ?P¨8×®›h?uši»îø®?oÅIù°Ê?ïWCfZ
?ˆŒ3‹ï?e/Ù÷fs?guaBÙ?'q¢±@?†ö÷}+x?ïÒG	¡5è?R½mk¸¿µ?H•Õ|Þ¢?+佡Âû?sÉÀ}/þ?Q ^\'4C?ïšQ­q½²?Ž€ß(>©?_³Z:'&?Z\;S3ø?…u)fš''?ŒU_Éb`Ó?ïgwوûo?'€Õaø–Ë?VCW"ª€é?^ñ øÒ¾?'¬ÏRúS?'οöbã?îŒõÁ?–Ðøñçæ
?r=,eI"ù?sáv¼ò§Ž?¤öy¢
Ô?•ÇDöʺ2?ï~æ+‡\?r™÷I^T?VçÍ{•Äð?Dƒ.ƋJÄ?i{`÷Ñ-?qµFéájAGN4FGL J1607.0+1550¿Ýï"žKÁ0@E³ã*cÇÀ8•Ü¡u0À;͇®µŠ'@{/bÄw@"mH÷Q?¢:ƒ<=¦‡?¼i€0M6@80yþÊ@g~igw³?ïÈtþ¯è¿Þî|µ]D¿äYÝâìпäZÿ**¿¿çp²Osڿ鿞EÐÄ©AGNbll3FGL J1607.0+15514C +15.54?èlÙãò¿a?À1^i9Kó?¼:Òc傦?»X½±Pð?À//<¬?³¡Ð=ÓFÐ?Ó{™ȽÉ?ʪmÁs?â°1-Ÿu|?ÌfC‹šþI?¼á\ý?²îDy>?äPîê{UÙ?³"[Pº€æ?ÃӏÔÉÆ]?«VŽI\Õ?Ê贃n£»?°%o¡¸?Þû˜ÆÏ¡'?«À!>ú"?×âì\<Êi?®ƒÉÖPø?ÂBõ¼é¦?šÁ¨Í]Ð?ã8d¨ÿœ?Á€â܌;?«ûû›cÀ'?¡šñe5ù\?Ö\ÃÊù?Á`y	3?£`€&±?îs<Úô$?çcáÌìµÔ?ÊàäwÊx?¿š0˜N?ÿ?»öÁ«Â?ã"M?³'0aë¯?Áõ¥zÀÕ?¨ÜŽÏ¥¿ú?ÐÝ+¤œ=?±¥Z`ðv?уƒzæ?¬ïQz#»$?੓ďÞÒ?·×—Ö\)?ËB©æÌZë?­C üæíMIXED4FGL J1608.0+4949¿éò"@äC-@G0dÜY2À;d»—cYÀ<ëëºÏ@Œ¨N"5ý@'<?ÓÞ>ɔ^?ڙ‡%"Ï8@8OLnmœ@ék'…?îü'"ø¿©˜ P`¿âôu
œ;¿é5ðè5 ¿ß²¢\¶º¿ïýÿ!]ÉAGNbcu87GB 160630.8+495728?ïâ#Âì"?€¸`'±Š?E÷££PW&?QêI¸g¿?h^T‹¦Ç?}V›:¬ñ?ï¯0"ÈNŽ?€4gÿ%?]i'¡-±o?d\±+
¤H?€†µÒçnf?y)xà>¬'?ï;/ù9^¾?ˆFé|
 /?v‹³ÛM?vÒ/=×?'öóÉÐi?"Ù?}™/?ï£K-È1ª?e¥v‡Fáá?f&¦üd??M'IÂ?£ŠÑ°,r?cÝó$Í,U?ïÅ3¤®[Ú?€ôfachI?Xæ16L!?Y3ÉÓŽ?w,¨Tõ\,?~ÂØô?ïô¼Lne?ž]‡Ä9?q›Ñ©Áµ?g9)×;Ô?™zt˜Ì?™9ˆÖ¶'?î·<úm€?"‰ÖnfY?‡B—
Õ?€g¸÷ïœ? ­[KãÕ¾?mœ¬Ë~?îÕUQ7¢{?†û¯rЫI?x{˜î)Œ?lEìԘ3?Ÿ6o¡Ð)6?†pÖñ'¨€AGN4FGL J1608.0-2038?Úñ(¼Œ¸¶@6'¬dwxÝÀ9㋘O¿À<hXÓ×@…€flÆ}@ž§b¯ø?¶‡a!œÌ™?vàé—çE}?Á>ìdl¼@õ+ÆWgÆ¿åù§4ƒ?¿âEB;å¿âsáxU|¿ÞuÇ,yÜ¿åOv_Ø­¬¿ÕqEiÃAGNbll3FGL J1607.9-2040NVSS J160756-203942?ï͗³t•?{ÈáRGÈ?P܌ýøM?@ÊÐfȳV?u0€e¿ò$?zkSm2Ûç?ïچž6®µ?q"Þߙb"?F×JýxœÂ?QP°‡Gä?oÏN–x?lKà€-l?‰‡v?}|:㩦¹?Xé-ì°ò?CXšZàʟ?‰¼x¸:]?|ëHK:ì[?ïq¼Ø«?i_þ±\?aû?g¦,Ò?AïÑCS-ô?/{š_z?gD‡Dˆ•B?ïšÁeVÇ?~³Â¸í^ø?`¦ø{?TŒ®¹n3?…%û•¡¸-?{å—Pîu?ï'qâùèl?ˆ˜I—¶†?T4ÊW¿"?añzÙÌ ?ˆáÀ°Ñòæ?†²Bîù.?ïœ¨M?
ß°hãÐ?fÒy§é@?cW¤éL"?œDN5Z?ŽÆÓÊ©L?ìP~P?†q¡z[Z?w|øM?`…l¢}á]?¤•ï:ìØ3?"Ù‰ÄËAGN4FGL J1608.3+4012?ÞÍþâ.ïé@GÊʁ˜ñÔÀ;‡³-¿UìÀ<î™
'¡/@'0ÉKó?û(¥U~Ž?àÒèÛ­e?ᚮÂu°Ü@Q¹eç»f@Yuƒ?ïئõ¢¯¿Ú´ÈÊÍ.¿â›W¿"Ç¿Ú"K©¢¿ïÿûÎBÓ¿ì—æpâÁ+AGNfsrqB2 1606+40?ïviø°ð?ãŒýÀ:?|Ÿ$ÝÙq?œ&øOM[?"ïtzLä?ƒi+tb ?ï'Â9öÆÆ?†`Í<Œ·Ú?h¿íí4?okìœÿµA?…MðFü/?€æ'­Þ"R?îvûð"j'?˜åGöla?'óSÛZ•^?Kr¤u0?ž-.¯w?¦»?WY?ï\æÿd4ï?o
¬?wSÓþûŒ>?bûéI•­?V =Ð*?j"R¶f³?î¿3èB|°?šg÷àX?ÖÁ`÷«?'%‡¸–k?—Ci-¸le?'ÁåÜöã?î™øQ_îþ?£Ò‰ٖª?ƒªÙc…J?'Qþ,ˆ¨?¡™Ð1loÑ?›Xÿi?큐ªÌ`°?¡
­Ý7Aú?™rUgL?'[ÓâÖÿu?«-ÊËb5ø?šûà×2æ¹?îªÒ;&_?‰"ì	Î?{5&Y±NN?w-Ò¦ùz?¡ì7ƒ÷\H?…îý–q°—AGN4FGL J1608.7+1029¿àDÙl~"—@Dg7âÅ\–À9($}ÊXÀ;æÜ0@úñ£Eë@©æ~Nº?°¦3
9?Ä^DC{Õ¹@Ęވ¶ó@*
díj|¿Ë™à¦ÉWø¿ä«±^²<ÿ¿ç^Á÷†´»¿èÓØYÉ¿ë†Á½¥¿ðAGNfsrq3FGL J1608.6+10294C +10.45?ïÀV¯³ë?sEà¿/ñ®?vthç…ïÈ?oußќuX?bÀá	?\tÛs(?ïÏ:E©µú?x˝ò©5?Lå1—9­?VäÎ)f?tÆ7ýñ?v{á7"ñ3?ïI˜L4ˆ?x	äÁe?xûüžú<)?}žmq#*?÷Rqè?ŒvcW¿äÅ?ïßô¥aƒ?PŸÏÖY9?Pɀgpˆó?6'KØz?g¦š'má?K,E/ø.š?ïŠ×
\MÎ?'ûñˆ¥¢?'B4g—?y˜Çœj9?vXÌÒ9?t'õG¨%È?ït†ý¥!?Œkbf¶õ?`ôœ˜±Ä?nš®$³¸?Ž¡X7¡l?‰¸
..$?îÛ^'—b?—¡_|?â
Qã	?ƒ-ÜkU*€?›®O.2?"é«_&ǎ?ï£4ȉœ!?o/á%;§5?iºS‰°¿?VOl˜×Â?€Ä*4«˜?i¥ÿó†›AGN4FGL J1610.3-3958?ïÍqZ`HÀ@!îÐ,ӞÀ8û²êòÀ;hâ·Ý!@O=yÞo@rÓA[#?´&òH‡X?¸'­¼ç&•@| fèl@n'ÏùR?ïÿ1£æúu¿åaRàø}Ö¿çm͘¤§¿ç㺺{'q¿æ%ہp'õ¿ïýYÝl[AGNfsrq3FGL J1610.6-3956PMN J1610-3958?ï¹òƒŒ?¥v$ÀñЧ?6ß6±W™?T §—"œ?ɸÐ&ƒ?¤ÖO¦ˆÛ?î]p¥ÑÙ?§¦Èjã.Ö?nqÌBÝ£ö?sÀW5Snq?¨Fü/9I:?¦ZezxÚ?î›O@ì?'+î+¨`˜?y6'þêÀ?|.{#-? ¯x­T¦9?ÃT<¾w?î'÷ ;'?Ì吃ìl?‹˜Ldà…?h®m«E?¦šz÷	dÂ?~#"¶Õáì?ï`›W)]?‡Kˆy¸?B~•Ýgâ?7Ffä_x?"X pœvù?†ÿ(ýjÈx?뇰F•vÛ?¿o8>'>?ƒÇî8#Õ??ŽohÝRð­?À¤À'ç??¾‹˜"Îî)?î/«Lj?›àÉ,O~?€Þ 
THS?ƒ+³à‰A"?¨Ø-L@)Ï?šL<Çñ¸?ë?žæ?›x+ŠÈE?¥á$ú_?ˆ™üuã°?½=ô¤¥?–±á|×AGN4FGL J1610.6+2414¿ïý4äcAn@F©A(¿<À:ŠŽ›8Ö
À<W[ìà³@ýI¤¹³@@ëGâàí?¹Áµ¢®Á¿¶[¬¤
eï?û=L¬€üë@5ƒo‹©¿áÌ=]º¿ç+{؃¿ë"9`÷ã¿Óe="[¿å£ÚЛŽf¿ÔÎ9´V´BAGNfsrqB2 1608+24?ïq
ôû•?'lIJµM?`Æb>Rdì?aéåùLê5?‹ª:)©?'\w{ìÈ[?ïÊÒ	Ýq?u¾ÑøµÒÃ?OËt¥FàŠ?Yä´ÖO@?v'yþ1h?q=8W¥Òd?îä›x?à?'CÕËÌ ?i¡QLz¾?q#Œuc? 9é'Ó?'ŸÔüY?︧gÀÈ?a"Nû]}b?[ŠÉfÎ0?EþYÕ×Ln?|ÉÅë¸ôs?^¨ï\…?ïŽÙ™†F?u^Õ7$f?md…ÊŸ?j¶ë—CÐ#?™!"ͳI?›éï¤;~É?ï]¨¼*ß?'¢Ò¦¡,?_ÑAÂhRù?p{rH'#1?'MÔZpõó?'@À"¤+?íÞSsf÷?Ÿ^H§çú ?}ÎØB/P)?'=AI	€?®eÏÛL?œöS5RX?îøhV"ú?†V)otˆç?}yü&sàŒ?qYöm9|?™"v1D!–?ƒDŠO 
	AGN4FGL J1610.7-6648?î}Oó¢À&EÌBcQßÀ80äÅçÖ>À;]C¢ìÿr@m‰'8Ìû?ùÑb§•?£rRØ¿õ?¼fý4ÑC@¯Â¼¨'[@Ëïž]ù…?ïýÆ¿Âx5¿Ë‰ g¿¿ÓPÛ$Sql¿ÒjCÒ ¿ÚÒTჾ¿Þ(ƒÕ,ÃAGNbll3FGL J1610.8-6649PMN J1610-6649?ï0ތ½¾?œä)e1?f`ŒÉ°ÅQ?"dW5 "9?—ՙg)?™Ç:Z§'í?ï7ûR'j?¤$«weÝÂ?iÃ&›Î:?|¨Ÿ ^¤º?•Î}HwŠs?£
'BD[?î>D?0R¿?ž"01é4¡?'TEàŸN?'"Cª?£q™‰9`?™Ú]Å]5É?íUñF(Ù=?'FtŽGV?"Ö|Ù,r?iëN&°l?²µ¦3"§Ó?'7ksã¥?ï5"‡Ð€?šO¾ƒK?ayßð¹µ?eY&ÙYj?›ª¬KUœ?˜ö"÷gbâ?îJz³¶Œ?¸'³M—.þ?€`z[¡e?ŠcQ' ¯?«c9Õ÷‰]?·°þI£`c?íé…p€W?¢ù^+R•Ù?>uºýÐ?2¡¸­ù&?©˜ŒŸ)? W¥ÕÓ`Ú?ê'Éý »]?§¿æ$v?'"Ûž?|~b[ù?Æ<§r—š?§œ)ÇÈ­¹AGN4FGL J1612.2+2828¿ï
z@FóI{t¥À;j€G¸ü5À<É~#òM@ˆ0,–?þ6§¬Óª?Ó6^á·Àv?Æô$j Ü?òÍ…/?ÿz·^P˜I?çÿMR8¿äwý''i¿ÑE†\{&¿ãþœÞGžz¿Ö`ŒÝž5¿ïÿ®©ÌAGNbcuTXS 1610+285?ï"¿
‡?áPXHÚ?c•-w…?k`Û°¿ú?†2ªòé^V?‹•`ëKiÀ?ïV}؝æZ?ŽÎ&lŽ9?pèwÙn†?sÄ0ÆòBR?'ÊÕ?‰Z¿T/?ï>™ñá·É?…ô/#òÿ?kê-¼—?k-§0¦?"¯|VJ‰?ƒˆŠgÔW?î¿6	DÞ?zӄÃ9ù?p¶ö
.g?WrtV‰¥?¡õÝ®š¨O?xÌg*qD?ï!«Kü5y?•tä±Ú~?s	ÁN±?[?k†k\Ä?—&(Ùt?'½ÓB"JW?îz·ŸFµO?¤IØcŸZÐ?zÌ–l1ç?"©à^†}?¤ûœ
ÅÓ?¡úÇ7Ъ?îsyÝÅ?'b'³pè?xïH›!öt?u8?¤=1?¤ÊåÁ
Wå?ÝŒ¡*á?ìc£ Ù~â?˜*­Pü3ý?~5|á"0?p°Tù+ýk?ºÿ‹)Ù0?—‡ÑÄN>AGN4FGL J1612.4-3100?î³DÁX­õ@-P¯>FŒ¬À9a³õerKÀ;ÐôƒÊû;@µÉ¢ö»?ÿiðÿ±üg?²ÿÂÊí?Ár^—:@¤[^Ëgr@7ºC³3?ï÷T?NÛ¿Û%î;²]¶¿ßö"ºÝa¿ÛüÚ\¿çÄqê('f¿å	BsíãAGNbll3FGL J1612.4-3100NVSS J161219-305937?ïãj;:Ç/?mhçf«W?C)C–áR?>–‹Um?gËsø'z?kвŠ?ïј¥—˜|?zò}qT?PÌeùŠ?Z¸W ~þÌ?s"Õˆ¨É?u{kʖ4?º/§?ëŽü¬?oö
¥êfº?uÁ¬úFÈ?…×òڛ?},¡À?ï'3ó'K†?gx	AîE?d.u ùYÓ?E ßlñµ?Šge²ð?dþƒØ'¶?ïލìÐ_?kéQê$Ù?NL•©*©$?H{&ؾ¥ƒ?ißØp®Žª?ihØš7ç?ït<ŠAY^?'ÝZ–ß?eáCk(†Ì?sU0úlïÍ?xŒŠ²Ø?•TãC­?ï7QÈʉ§?ŽŒ"u'K?~œîÉýˆ?¨àLDô?'n¢¨"'Ñ?‡K…U
$`?îÆQ+§ß¿?ƒ‹'"•œ~?xü[È0?b/q"? {aÉiX?ÿ=Ýg™AGN4FGL J1612.4-0554?ï¶UôB @?C«CIIÀ:pHD<oóÀ;÷žXE;s@y5ËéÍä@­"'±È?Æ=vƒ? ŒÂ_zRÆ?Õ\cÞл@5H
æš?ïþ_ìÏ¡"¿Ö†—^Uö­¿í´4 ½¿Ó#>ÿP3¿á‡£,ÀRk¿ïÿý{ÁA~AGNbllNVSS J161228-055752?ï> j6]=?šE¶'ÒÏ?Y/,£Vš?Y€K¥âª?–¨ÿóR¹?™ž¢è'?ïÚ]ûͅ?p\ôiø*ï?E7XŸûí?S;m@è?p*ØÊF_?j$¢æ?ìµh
ÎZ?¦'8	-f›?Š  B%ûx?ˆÌ^µ:'?·»Ä›Á?¥‰ŸUº)"?ï¬ÎQ‡1?i±ñÌ*ü?WS¾Étí¯?BûLá]ê?'
"'¿©ý?gRÆúbu®?ïŒUR0¾?šqÜzå…s?dû¯Q$x?jHÏq–?šŽÿoˆåG?™ ¼â>¼
?ï™å»J'?‡/זÑÔy?S›Ý#ƒ©?^þ©Sw?‡>ì¼æ­?"Ç'åÞ?ê Æºl«ƒ?«-!‹Àèé?bÝύ?•p@Äf,ø?ÁЉt!SÑ?¨«ùRóµ?ï
\÷ý¨?†©…‹Ié'?sD®˜÷¹?d¶Ì(O×?™'OÜé‰?…Ìée$kAGN4FGL J1613.3-1907¿ïÆ	t ¢@6®g¥*ÇTÀ:°Ä±uXrÀ<‰X=@ fÔÜeÇ@™×ºf˜»?Éé'¶Ó;Q?¹hìÓ}k?Æ£ÌùBv@ºØØãÁ?ÒO.¦Üx;¿æ38q`•l¿à㠀þî¿Ùµ
¸A%¿ìÀÊ*Ü?Ó㻹ÿìAGNbcu2MASS J16132720-1908364?îGel–VC?ž·ž™1	¥?v]?W£ì?fнê~/þ?¨¾Hx–t?*<ûš%í?ïlèþ~*?ŽÉCŽÍ?jSO^É?núx="³J?Ž0ì¬ÈÕ?‰1n`PÊ?ît€¾^þq?˜ÝUAa0?Ôím¯B'?ƒc~9j?¤B¸¼h‰S?•?Ø^T?î*{Ö)Í?ƒÓm™l=b?l-ìuRH<?R‹Ì'Ÿ4?«•cÕˆ´?ƒqi°<?ê€çqœX?·èº•ÇåÎ?ŒUfžKƒW?~3"‰p@U?Ä7ÐÚè?·>ÚG&»?îÉÓö.<v?¢²òëvY?q6p¦B‹Ì?z°Íè«¥‹?¡;ò‡b«?¡jråzÄ?ìŒ4аöÇ?¤+ ,ZÑÞ?*ÿ¨¯E¯?†0ö°›ï?·øù…ba?¢¹QÚc?êNÁ×b? >‡ËÞÒ?'Y<¾–ÿ?pP¨ìÍ8"?şh÷
¹? #Öà&9ÞAGN4FGL J1613.5-4225?È(̊ª
@H)ŒÁDÀ:P#tƒÀ;'I:µL@czðáÿå@€c?jy?Ñͤãú'?·aÓȌv?ìÿMB}þÞ@ˆád3†?¿ïôµ´'S,?ïÿÚáb†¿ìõ¦n"¿Ù±ÙŒÂÇ¿æú"ˆ¸¡¿ÚŸ)ÜvAGNbcu3FGL J1613.4-4222PMN J1613-4225?✏m-«?ƈ³Á½	?z–IÏøv?tªƒ!ä%Œ?Ú\ˆ™8˜?Ƙ­ãtüN?ëBתî£?¹«—Ä"~‰?{VkhüR?ƒmk0¸?Âíøý"z?¸NP‹.?ã±ÝÓãÊô?³4÷¼Ü?ª\Ì
þþö?éi‰³'?ÕPª×wy?²lɯpw`?íe'á&?'ªããfX?{ŤQ'ö'?^Œ³à G?³³xÈ&?'&÷l†Ü–?×nh0ž‹ú?ōÜa•FN?˜7#´Ž]>?™²Ý²gÃ?ã‡ÊC@Ù?Æ.ûO0Á?åd‹"éÏ?ÈÓōFË?'bÄèŸ2­?¤™·ѕ?Ôžš×©—?Ç®³7¶‹Ô?Øwdþ\g?±Ž÷zn‡Ò?¸'»¦ß¨G?¦wšþ3ý'?à´$X`$"?´WY™~‹?éÕ:7ÅzY?©N)´‰m?Ž@…¯ãÁ?{WÍÇ Ÿg?ÆÇÎ5=á?¨Œ'ýdÃMIXED4FGL J1613.6+3411?ÃNJ°þ:-@G0Nø‹—xÀ9*E†òÍèÀ<DÊPñŠ@£KëW@Y䒼/Ç?¦»®—WŸú?Ÿ–k;ã0?óFÌ¢Ûa»@Ñ´ì–¿Îú"€'ÇE¿áýÔ þþ"¿æbE'Ë¿ç~b †ˆE¿à'Tჾ¿ïÿ‡¿ÒhmAGNfsrq3FGL J1613.8+3410OS 319?éÌOßfWx?ו$#éG?=´…ê?b©²óc	?ÈÀ1¦ô©"?חr±?ïÖ
³ûMF?p ‡d+ÜN?F2¾ÉÔ§™?OªµŽÈ?r2Î)ˆUu?jÙ-ÉÏ[?ï±
?vàébM]Ç?Y-q`?bSð|†6±?€–4'Úkò?uKä\,ô?ïîî"ó˜?Cý*©·¡?L'Õ#/Êf?4H<D´®³?Uš¸«•3?:Ó5<Î}9?î,‰ï55?Á^(T\ù€?HñPˆƒD·?D
i"ú6ø?¬Ó›ÈóÏE?Á`ê]xÎj?ï|G±šlR?‹/ž4Ÿ?V"ÞÄk?d¾ð°Ÿ¢?Ž,Bÿ*Ø?‹i('l"?ï{>G8xÂ?€	8EO–?aèKEàR?aE£=&e?Œ¶[WzÌ`?~:ÛË{¿˜?ïÐ;¡!_?câOè_5?dP?#Ԋú?Tšï3™Õh?kt#Gh®o?ZM7S›ãíAGN4FGL J1614.8-0850¿ám×*b˜ë@=É>¢ÒþÀ;7x"væÀ<_"\h¶£@"җ֜Y?ý+G&/>²?ÆeXŸSl念)f€½¨?𗐪ݎ¼@~I‰¶Í‡¿æœ"¤?¿ìGðI´¿×ôƻ栈¿éùqÁ
{꿳Ce/"§ð?×â•@ÄkTAGNbcu1RXS J161443.4-085130?ì]*fl+Þ?Ìɲ¨«§±?CM|o;i1?K¸#€ŒO?¼ðÓð‹!?ÌÌ{¡¿‹y?ï)ßBMàç?Ÿ@ƒQ#v6?uPÃU…y?xHìÐôµ?•oæÞ?Ã?šž"t±ô(?Ķ¹÷?•©x†
P?\L#YÍW?g I'ç|³?¤ÕB™ÛóV?•xt",2?îoŸÞé@1?•"¥4a?C÷ÇÒI?8Q}õ­Š?¨¶%䒧'?•)gˆÌ?ê;g;ÅËH?ʦoâï'?S$màê¤A?S³ÉAç#æ?Æì5òfv?ʝ–QCG0?î‡W\)Ä?«{¬~æŸc?t Í×mƒ?"ƒƒúî?±?¤ú`Ë:×?©›eßÓ?ímWR»þb?  +>~28?hp
	ö?p—w­	m?³ÔÉé''`?Ÿ‡]
'C?é/UN]?·ñŸâÃ`?aêM/ðrî?b€ÞÝ|¡?Êúqàþ?¸
ˆ¥°$AGN4FGL J1615.6+2130?ïò
Ãl?³@E¸óË>WTÀ9ù9&BÀ<?k@Àºp@˜÷-žsÉ@ëÏkn
?¸aöKKX?¡¶m嶩?áMp€ñ'@\"òB¨¿Ã"ïCDMb¿è8ÁצE¿ëhÎUcä¿ÛÅ0@'/¿êÃJ¢»K¿ïáñ¿Ë]AGNbcuSDSS J161531.09+213011.0?ïöº.d—Y?Héƒg?5>)'ôŒS?1_€Ríô?Jx1·f$†?C£rüaÖ?ïÛ+	nØ?p†ÌDŠ?E%
è)Ñ?Q ò2^?o‹cÛ^?kÖתXÔ?ïé~֗?†A´îCEù?g›-:DMN?r?†%
§?†Õ	/ŸB?';©Ù•£?ïêf펨?FO¢ú|?Qp…
Bv?81ÓЂø-?Z´JdÈ?@X÷#*?ïòUn¶/ì?RçRþ‹Q?@vo•Å!`?5¡3H	?SêÐ)‹Ý?ORˆ‡|L^?ï‰Ââ"3?‹;:sn3?V¬a11í?b˜T3·N?Šé0®k?ˆè*jD"ï?ïI!̔ª?‰RÙLÕ?jˆ5˖Oc?mÌU虣×?"ŒÕ¢ªÙ?‡|X¨Ò>?ï¾â%F?g\"åu?nèÉܛ?^ƒ¤XpÃ?q†ÞU\:*?\bn‰t"AGN4FGL J1615.6+4712?¤g~
}ë3@FÎãK"SÀ:C{À<‡)éÞU‹@å5oùb,@GÇ$_¾?µî@dô÷8?¨f*ßÛ%?òŠFu/W@Ÿ´Ú'³ ?ëw¨¾$¾P¿Ñ´]¸½¿åMI"žˆ¿ßéþ Õ®¿ã&óõ/Âe¿æE£þwiÄAGNfsrq3FGL J1615.8+4712B3 1614+473?ï虞™€?S¨RJ¡Î?B?€Ü`†—?1a{<¸}?bրþã¸[?P¶±•¬T¨?ïԻ̧ìv?sâ'ÕŠ?I¯×â=A?RêQ—ø.Ð?rnc'x÷c?o¦àvÇ5?æò	?_ËÜw8Àl?S8kp'DL?<Dzš^k?yé£ËãJ?[}Þ8k< ?ï¤Û_?^B?^Å8öÈ?s{SXý¨#?NöÓÐJµ?züé¦Ø?Xó%6P?ïÍ÷µŒFþ?aߖùÚÄ?Rm¸G35,?@ O–Qà_?th·$ •?_œÜʑÎ:?ï{0Š-ã5?Š¯ש?[öæ¹ûic?d¢æ†ö–'?µ­mï™?‡qàÙÿM?ï™,Gõ?q"}ԓø?\€F/èç'?Jÿñ$Š ?†$õ­Á™¾?oH­ý—"?îú§o´Ý‡?}.´ˆ²;?Œ¼]?«y†?nÝ|ÉZv¡?'LãpmÊ`?vªÔà0AGN4FGL J1616.6+4630¿êp¯Nÿ¦@Fœ¢ß"yÀ:ØÐi9~À<-\6@øÓËCµ·@±PÚãæÅ?ÅM-šÂäl?»þÇƨ›j?ñoxäl-@CP¿Ê^ªïj\¿åƒ]b[¿Ä¿éR,†pÈ¿ì2àÈ,T¿ïùÕyC¸¼?ïîê>!βAGNfsrq3FGL J1616.4+4631MG4 J161600+4632?ïô íS‰?MÿóiÎ?4æuóHñ?-!àêÖ?RÅ gï¯?JHî^O?ølҀ?é•ïæ¹O?f‹ÀT!Ìû?z?ýï?†­Õò8¸?ˆ¾Ž!"šï?ïª#ÛZî?vŽåòöʨ?^ÈBº¿Íï?aW­¹%Ãæ?ž֜ˆÒ?t{8èwJ×?ïË(–æО?]ùo®ÀȊ?V¿öOPô?@3›3‡ÌÕ?t»¶Û7?[F'u?ï筜8ï?`²¢,wo?DTÖcQóŽ?:èaŒù8ÿ?c=-õ"Î?^¡µ¸¯A ?îÂr'ö·N?¬z€Y=?sØÆÿNs?'²é™Ýœ^?¡]¾ð<ÔÍ?ª©¹ëQOÜ?ïU"oUoÀ?"LÞÑÄ?jdì7§`?n

Ðâ¬?'ô•ÀP{?'?87q‹Ô?ï$•ÖËÌ?"œD+Äx?wcdÈVó?eL°ÿ²?•"š™)Ú?'q«ŒµÙ_AGN4FGL J1616.7+3327¿çS
g+Ö@FÖÄ`퀡À;ô/eƒÀ<¯'ÎÉý@g(<	E¤@:#|ÜÊq?ÒÛ<'¦?̍À‡ïø÷?øì#>Éik@vþöj«?ºÂÊ?~Æ¿é"i†¬W¿·™y¹)'¿á`àpÀ¿æëg@ò¹¿ïøUFƒrAGNbllNVSS J161633+333043?ïÈE¨o?qqN*<5?Wñ↡ˆ?LÜTBÇÛ?uà³+_ƒ	?nÄZô
	?惘F´"?{"\œð²v?Y(ùGÐáF?]P­»¬V?'T?Q‡C?v¡¢Idü›?ïuòWmF¢?v‡8£Ÿ~Î?duŸåÉ(?TÌޔÇ4?f/³‹ƒ?uRã?ï29f[²6?p0¦Ë
F×?qxf¦Ï£q?Qå½s8gî?•Z¹"Òm?mu°ÜƒZ‡?ïq¢Õ,—¹?‰Âm¶,px?hm3'i?](æë?{æêÖJ?ˆG
ƒüU?îö5›E?–B\)·ò?mŒK.Oê;?qZ2#/Y?‡Ã0Ö\z?"S'ÏvÌð?îÝS7Š…Õ?‹Ž=¾ÿ%?u!d)ycØ?q(½»Sð?Ÿ
@4µZ?‰.7d´ú7?íÉÎy¹ï?Žm/Ȇ¦?€l8*pna?kϲÙ$T¹?¯H
Yðî1?Œâ+×tFAGN4FGL J1616.7+4107¿åగ7½@Fúù3]$žÀ;îgQGñÀ<ÝÌúïõÇ@p@'Òë@Rºà;>š?ÇFBšvØ?ÆðÀU?üª«õ¼°@I+®Ús~¿æÿb`ÈAο³ï(nß¿æ''àðp@¿ãk¥Õçþ¿êžJ''¿ïÿý¡UûŠAGNbll3FGL J1616.8+4111B3 1615+412?ïŠýš%Š?|ô†·ç#?uwö…O¯?k0[À*µ?'"ž@å{Ú?uÀtÒØ?ï–Qó蚉?|16*ÌÃÑ?dt¬îi¹Z?cĈ¢$Ô]?…NWÉ7
€?uÕØ-à³?ï6»äzÆù?…ÆåÝ36?v:*mAÅ?t]ÜßyL?"™ý-`?']âÝ#î?ï"peBÏÞ?rÓ¾Lô~?‰;ùdé§?f¾ï¦Uê?Ž'í¢æÏ?o$¸"%-?îÀ¼µAY«?"Ç<BH?Œ¿È:=~ì?"®ŽP?™ˆ…<mÙ?¡™åa?î™qKzZm? ï/¡xù ?z®²0Åj?|VYUJj?£Žüš‹?ŸÑȯ譬?î,@ÿéH?—ú¬žçW?Š'›ñСÊ?ƒ€"¼'´?¦›Ic˜½?"œˆ{4
?í'õ}zÄ??䂲2©? xè1%i?ƒ\äYsË<?§X›cy]?‹±˜·ôAGN4FGL J1617.2-2535?د€CºÈq@1£Ï_ND1À:a-ñªÓÀ;Ñ}‹Q@ïՃ)Á@™ð^¢LÇ?Ð;¹eç»?×ÑË9NÖ'@¢þ'Q~x@ü¹"`ʛ?î´º𠏿ÑW³°œž¿áÌþ ÚU¡¿éÒI
{¿ël‡þ¼'¿ïÿþÐñAGNbcu3FGL J1617.3-2519PMN J1617-2537?ê|½¯ÒÉ?·n7Õ<.›?²6Ã_"?¬då·ô0f?¹ãûÁÆ£,?°Ó/¿»?둒:Äeå?º/ð•v@Æ?±5Ú•Ý?° ïÓ{×?²="D.|?°ùònóž?è.zªsº?°'²Ï¿~?µ*ï,á? º׿À?Ä°¿÷"å?¨Øê¼qÁÖ?åÄ«~?î?œÎô/?¸f£
þÉ´?Âö!ic?̺¯Ë¬ˆ¬?šïU?ä?Æn[IÊ?ÁF'F†?Ä2Œø©þ?·ö]­ÄÄ¢?Êû³¹š.Ú?¼o`'UÇ?äz¦ø…jì?Éj¹XË?ÊÕ6jl§À?Å·ÔpI?Ã@-³}¬?ºæ›ÕÞï9?âzWûG<2?´©­²Ý
Ó?¬¨0Œà?¨.ÌJŠ¬†?Ñ´ûñcÁ,?±Ì¸Ö7ê?×Êa¦@χ?¤ïb(21?ÅúvWŽöí?¥¥ãùH³?Ý8c/
•Á?¨Ñf1ÐgMIXED4FGL J1617.3-1513?ääÈԒ
@8†Šar
À;Dèg]À<¤Ú/­m@ t‡t~8?ûÞþ'¸«®?ÒÃöúȳŽ?ã$ì^¥«@
ü«>݋a@b§¿÷ý?îA$øÝÌÏ¿åwÿ ´•ô¿Ã"žWïU8¿ÑM²¥Ú¼¿ä·Z¿êU¿ïÿl\I¬òAGNbcuNVSS J161713-151058?îÜ.–/E­?'Ršr*Á?•ÞÊ$"ø?‹T£Ä‹wÒ?6ÆA–˜ö?'uƒñÈ*?ëá!iÏ
?¼ü_Ն7p?³2É$þel?¸¦{ÂÀš¿?«ˆ[ý®v]?§kÑy¼î?ì܀¡')?¥ïŽÖŽö?§˜ÕS¢ø?œo}Í?«']RÖn?œqºülñ?ç©ê—‹L?¢{‡1xx+?»‡Ä¯òÌ?™u—ÉÅ7U?Ã×Á•Ùh?›ÃCÈ=N?îŒtÀ?žì#²À9Ê?¢ª¶¦›?—ì]L;‹Õ?–ÊÉzºÈ?",›Š!¼?å›Jݍ©?ÊUú¨¨*V?ÊH؀ÆJ?È"Œ,ô€?¾–éóƃ)?²zGwkz?êËé"¡s5?®ÙT¦'ª?²›9šR ?¦3=–¤ÌÇ?·}OÆm¶?£Çzp'÷?ݼ(F3?°1ÆIƒŠA?ÇüœÜwÃ9?°%E¿|Ø?ÖE‰}}ëN?°›N›0¬øAGN4FGL J1617.3-5849?￱'ÍÀ¶R7yÀ9>Ì?ß À;"ˆ9@"שÇÁ@ŸÜ>Y×ã?µM16-äj?Î;y}ÅR°@Èa-A'@NÔ¤\–?ïÿ¼®q—ó¿ãJ;ÝüŸù¿æ^:é
5¿æ2qôÆ¿í"t¡'Œ_¿ïýÍ ²<©AGNfsrq3FGL J1617.4-5846MRC 1613-586?îýي~ ?"T¦w,ð?"ü^þ7?€,¯<m?–<P²,ßó?ü×íÂYº?ípã\R³£?³XQû2Vc?k[y òR¿?|¬ý"ñ?³ž	Qù¢?²ÄŘÈ[?ì¼E¡2H?¥ë­Q³z?¢äC[Ö\Ç?šX«ð$?°«¶#Ádà? 7&ßr)?îx).Írå?"ÿtŒ"P?‡ç8ý°A?m–ä2ñü&?¢ƒž×,]g?€Sµju¶±?íýã±wh?¢ƒCÿ¤´'?Ò¦©?ˆN[²Í*?¨-CCÇa?ŸBr}ƒ¶?é³äpNéê?Ä´¹\ÏÜ?ƒ?ªzëk7?mæÜo6'?Çüs–Ù(ƒ?Ä;ŸØçs?ê‡m'T«Ô?­h³U~øß?²zÇÆx€â?¢ÇÒ6 ?¹I˦â ?¥ã`ÑÀÁ?ëELøp?¡NHéL&?¤–GO´n?êŒ²G¾Å?»Œit&²5?œ…Æ™{zAGN4FGL J1617.9-7718?ç²î–2˜À2ÞM;òõVÀ8tvÔr³|À;²/,=u¬@‹Rùw$Ð@ƒ'?	*K?¡.—3M_?¼¸ÈúÃ@À‡Þ†2µ@©Ö¨˜»¿ÖýCãÅÝ¿ä…dXo,ß¿è™Ì$0`ñ¿èH*;<ìð¿èS½í5øà¿ïþRúÉAGNfsrq3FGL J1617.7-7717PKS 1610-77?ï÷|Æ¥y?D°É¸"ô?=-â[ÀHB?4›Rût~?CuôzC«?;Äv|(PÂ?ïäUCm+ì?o~ä&"±?;e'´:OÞ?I'‡Ó¢?¸?h>
WìØà?m2W¬ÀÛ?ï›À@"	?"W×ûŒ'?j
' ½Ôÿ?wߛÌóºØ?';€d¡?€'4Úd?ïè|™ê³y?K;ZwÞ?J)ü«,?4²t5ÎÅ?`øæù¤<O?Eåci??ïëæ?\Ø?aڈëU2?D¹ãI?>7˞`!À?^1$ðbC»?^1ÛpœÕ?ï°á–ªÉ9?˜["¨…÷z?dïAœM˜?–ٯʍ¡L?}€¼ð` ¹?óŒþû?ïr0ê·!?ŠÏ•Ç*‹?p"=ÍP,?|NCӔ5?‹*&ÃXòÅ?†o')ÐÃX??|1ª?l±C,ÆÂ?e{µ¯¯¡?Vp¯‰}¿4?w?U_ÀË[?f+h3$*'AGN4FGL J1618.0+5139¿¿ú3ÉlVQ@F8AVâeÀ:Žf$ø
À<ž0´Ó±Ã@Ua÷ÁÃ@†6Œs?˦>m£ò?Ìd6÷—&?ýñ¹KÈË@µ"Üž¿áÊ~ŸBP¿âÐ{÷È¿ç=xÁ‡Ê9¿í8Æ_ö4пåF/ßÁœ¿ïöØmAGNfsrq3FGL J1617.8+5137TXS 1616+517?ï÷…òÙì?CÖå4æ§??/õZõÈ?"Ú¤ÎÎ-ú?IîEl|)×?A)cf¼ê?ïãK9—ÙÚ?k!TùS€í?;£9ÂwÀø?FD‰!ƒòF?i@_›Þ—?gÜü¼?ïZÅÙàÔ?†"wµ‡û{?oµIë‰åí?oš¼Ž÷ä?È¾šÚÈ?…9S~oV+?ïõ·3?6CR¤R&?2IOä
+?yiEAþ™?Q5ˆ™µQë?4MÎ^‹ó?ïð¯¶Í˜5?U"fрÊ?4¯á-õ]?+é D]:,?YtšՅy?Si9*Ÿ5?ï–örsÌ?‹2g"
yÜ?Qj|½Ä/ë?\aùÌ_– ?ˆ܂¸?‰º¦ßœ@?î¬cʙ…'?•¼È¿Q?}Š§¹ñì€?y4Ü¡ó,¢?¡ˆn`÷4×?"Aºûã'?ïá7q©Ì?W'0?¸	?EÇ#o;V?3w™ß29O?iVÆfÓ]?U"),Â~\AGN4FGL J1618.8+0620?á¡ãü$@BQAAé¯\À;5¢é¤sèÀ<šè¯bk@*s6›f?ý™yƒyœ¤?×3Úé%?Ô¹‹|uqq?ûŠ'5Îï@ëyÙ	ññ?ï¶`^åh¥¿ï)BUæ?í1Ý'ãƒ¿àtž7ŽÇ¿è÷ôÎs•ú¿â.ó2'#"AGNbllRX J1618.4+0623?ïiæ!ãÞ?…AXº×+ö?mvý׌Y?_VÒ#w?Ž(¸T•p?ƒ&sæw)?ï—–rÑ6?"Fõ¨#MJ?dÕ/À)o?k︒^¹?…N'lü?~®Ãê&'&?îÑj‹ã?'ÐójÒN?sÏ#J§(?rö}ÈÊ3? n$ïÐ<V?'ß'Ù(SE?î×Q'vè?·•¯\€?pÆCÆj?`s@Œ#? z¯ŒD5?€y´ªt»Ç?î{âõ‹»h?š'_ì f?€'öf<¸?r'_ÞÁÒ­?¤S+
?—ü"õ©­?îé]:)è?¡ê8r¬'¸?uᙼãú?ƒnj¦—?[òra?Ÿ§Ä§)'?íœ0ûÓþù? žé$F[Y?';4Í?€-ÂùãÓ?°Ú°»ú5ž?Ÿø©ü;šù?íTkvPX?ž³Ú)Ûn?v&ÿÉÝ?pŽ·'Èë?³ü¥dyb?åÒ¦,AGN4FGL J1619.0+7536¿ä{¹šý@A¨ôàM/À:˜NHboaÀ<Ç>óZÖ@7*Èü@:dÜY?ÁØÍ÷o7Æ?ÛŽd9îí?ÝGåœÒ^1@D qúï¿Ò3 ~O¼+¿æÌè`§	Å¿âߟb[j¿Úa(	3…¿ÕÙôÌ.A¿ïÿÿ&¦³AGNbcu3FGL J1619.1+75386C B162034.5+754454?ïÐzÙ?iµõØMKE?Wr:hßM?P]ÖØèÝ?qæis9*?d;-'«j§?ïÔð›>?pwܐ{A!?E¸Ãí̇?M/%€Í?rÐÛUuÛ(?lsn¬™ó$?ïKދø-?tÃ㛠§r?cµÛxá?h=>àï?‹?'o¼kû?päB³¬Ž?ï­ÙýŒÞ?`?Fhüb!?`Ňðè?@¡ðœ€7?€X<eŒ¥Ù?^<¯»?ï'ÿ¥x[B?ßôˆ,Ó«?iO¤ûCúù?acÍe</‡?…,-oÒÆ?Šæ{®þÙÛ?ï…KB•ô?‡|†ºùùq?VO5w—§?`äåÙ±â?‹ðFyŒ?…°¢Ky8?ï^1þ?†å݇V?k$¯!?9­?eÇ'Î#"­?›é‰3)~þ?…™¦Õx_;?ïd'ÐC>?|s.,¯|­?vf©–2¥"?`ûHÉ
Ì?˜Å9_¼?{"]¢ÂíAGN4FGL J1619.0-8346?í¼Ö ]æÀ71qâ›k+À:õ6¥®zÒÀ<.Ï d$@¸½Mþ»‡@ú?¤Z½¼?ÉõMõVXÒ?¶s€wµ?éؽf'|F@,9í±?ã£Æ
•ê¸¿Ú•yyh¢¿à»²]µ½½¿èA•\¿æ;Þ§j¾¿Ì9\-AGNbllPKS 1608-83?ïʔZ.c"?"uÌ1ß²–?=L´÷[l?+W÷©`¬v?xá>ur?"p"Lޗ?ÒtÎÖ?~…m$(?`e—´\'?a{)d"úa?">	õÿûh?ym^"Ž[±?ïfðA'J?wéKk_àÀ?iaJäž?cmÒk;O?ë=*<p?t'ãxëc?ï6ý
˜€%?n2ê'mv?oƒu7U?NpÄ^bI?•/暈O?l¼ª2š¶?ª{¨?vBOw¿±?P¸Ž	?/E?BÊX)ô?ˆƒƒš¹06?u2îÁš7?îó)Œ…"Ù?˜§q>HÊ{?qYâ,W[?z¦$ÈÞiü?DUÝf©Ö?•ú"è!??îäbr2nß?ˆU¬Ú¾þ?vë¥0ú¿f?páÓy4Ó?¸ÈhL
>?…\{På=?í°1ðÌ?ŠÇ)µÐà?'œynf'?m«½Ù¢ó?°*áM^îÓ?ŠtY±0ÀæAGN4FGL J1619.6+5536¿í'PÆÛµã@E¡Þ?»×²À:†—¨'ÑÖÀ<³¯' Wú@5ÈRi¯F@õÀ[¥BD?Á7;ÀöTÛ?À¹‹§h6?ûIKRä©b?ûÜP§¿¶abEšh÷¿ä‰»j¤¹ˆ¿åê™ÑͽŽ¿æ]¤öÄíÛ¿éÜ5 uÖÇ¿ïý?ÔVYAGNbll87GB 161814.7+554307?ïb¥¨µZ.?…íÈ3Ϫ?r—{äªG'?j;†‡Ñ–?Ž
×êûš?'ä4:ÎÁÇ?í³¼Ê:4?«©?8?-TßÉÚ?›f0ò¢Zš?¦-‰\&õÍ?¢0éã,6?ïú|Ïß?ˆà$²*ÎÏ?Û{ä2?öŸ'èð?"ó/``€?€ÎÍF/h?í¸U߅Œ?ŠqvÿØì?¥¶ÒK´?"5́OŽD?‰6oß©!?|Ëm'"Æ?í§5_æÎ?¢xþüê?"â7ÐÎO‰?‹ôO§ðåÕ?«à½Nèa?žyš'	z?êÖºè	?À—p¹?k?±ÔÃÎ5(?µJ\R|ª?½4¬k>£?´ÄÒ%¨æ?î 'Am?™¯—\Ók?"LÆ?/Žæ?‹Uƒ_Þql?¦W›çÖÀ?'ȵ³MV?éÂD¹ÿ{Ý?¤Q´e"P×?½t7—=k=? ëB¹Ê?´y¢"é&b?•²ï'¹–*AGN4FGL J1621.7-1103¿ïmJg'E@:RÖËSP	À9ƓX6ø»À;ò­×>?×@‰s,Û*@ÐÈb?Âz	2®?ÊÕÊw]¼@7E«I@r 
´®?ïƒ=lr"¿Õh'{Mz¿äœ»sG ¿çÝ]Ó6¿ïóüQօ¿ï¢æÿþÓZAGNbcuPMN J1621-1101?ïÂhהZ?oa2œÑ!?dš>Šø=?[+ñ'/5ö?t½"ñ€»?g"š(¥-©?ï¿þ/›N%?~fxùÀž?\K*¦Q?f¿2DÃ?xùo?uUna:å?î¥HW4^?•¹4Xfh?šWùsñU?Œ'Hú~=?›‰Ñ¯Èuž?µÒd…H{?ïDaô'·Î?q˜'§Œ"?x¡í¶1kç?ZË ®]	i?'KEüù
N?nEéýŠÞÙ?ïÜÿØé?+¶·Úe?t͇xRù¬?p$˜gË?'":N¤ç?x§>$€Kk?ï]'þ̤?",kò+&?n-#ZhM?€JŒˆJ?›`2œj?‹ŽÞõ»«?íx,Щ·Z? ècõ%? -,¡K?–‡W/ŽNg?¨}Çç¡?™Ú´.)æ?í÷xóíß'?=ÁQzŽ??'ž!õi?z|ÙÇÀt(?§ý!³–áR?‹X~"C˜AGN4FGL J1623.4+0858¿Á½Ê>
h@BpJb#á‡À;a)ÄÀ<Œ«Ü'<®@ \<
<ç@V/Äé©|?È0§$G¿Qq±‰@4CºêÍ?ïü–ô£«k¿Ô톀¸!D¿ç|^?¦^#¿â?ü¥¬¨?±yÃeoñU¿ïÿÿ)@k*AGNbcuSDSS J162330.56+085724.5?ïFó8¾¯Ë?¤u1b&$}?…vo2?£øá7=?ˆÌ¢¿äÛ,?"œLùÄ+Ý?ïÆ^Òj#?vGýØÐí?J¡üÿç™á?R{åÞ|†¾?y|»õ\‹Ž?se¦^4Nø?ïQÛâ5â?Œ shœ?c²¯6YCk?fcúíÒS?›?n¢A€J?‹5˜ŒU?ï©ãÊ{tý?ež£ƒM3?CV³CÐk"?2bÏBùú?"Q¢74Ž?es¬Ärvò?îᘣûG_?¤Ñv¼¶.o?~Bû1ùõ? äµ"Õm8?œ<,¬õ?—ú{@ìn?ï~±Rë+Õ?&¤Ž?Tºž#Òz.?`4ƒ+
ÿ?¼W†:y?‹ÈNŒˇ?îéão6Ö?™µ¨< w?o¡‡·2s}?n¬îŽ%6?¬çILeŽn?™z±ØòÎS?îÑMË…?‡(®ÊÙ,­?]#Ô
ì!?TlÖë#B?¢
iŒ÷Ð?‡×R\¥:AGN4FGL J1623.6+5743?ï€ÉÙät@EÅXdE$À;÷GʚÀ<ÝxC½@b*"y@ca	/T?ÃWSùÒ>|?"ãpäTäð?Ñóêî?ò*}'Þ?ïèÙ¨}b+¿ãC''%ο؉ }8é¿ãã'àp¿ë|'Biñ?ÇÈ?Il¶AGNfsrqTXS 1623+578?ï\¯Â6,?ˆá!¼"û?oÌc8f%\?eˆ÷‡?p{Nf%µ?†oÞÆZ¨ÿ?îíZÞÓ7?˜²Í¶
M?ƒˆN‰#?‡^€{Öß!?˜…à…ë"?–Ð-Ô.?íü;E.?Ÿ&t;™¼³?ÆÛֆÞ!?‹½Ì*šÆ0?¨Ê"ºü_?™¹È)£U?î[å}ŒŒ…?…ìڍ?š­3>ÆX?}᪷£g?™Ö Û?z)ß^_/à?î¡#uÈP‰?š·+Þ|¸è?"ž¡^·?Öç{º? Æ >Ǎ‰?—ʀM_ˆ?íÜ#+ÿ?¯¬ëZ&s$?—ù<¶LK?œË4Ê¡Ÿ.?±rϹçÊ?¨ùõE{Z?ì—cŠz( ?¦ôy¬B?'']Ô È?ÖŒˆêX?¶¤L5ܲ}?¤'Á™I?댽CS"? ˜U0H?°F£GUD¤?—NE*?³XæÎþÊ?—,•ÿ AGN4FGL J1624.6+5651?ɹ1Fkk«@E!©T!ÀDÀ:΢Ç?ÅÀ<Åð®{©@Qœ«qÞ?@	A=?½¼ËLïò¿FÚ«´XŸš@cý/ìð¿ï†'Ìͤ?ïŸà¥Ç¥F¿è6¯¿uÌ5¿ßQƒòÖL¿à 4óý">¿â[7(‹9…AGNbll3FGL J1625.0+5651SBS 1623+569?ïêP	›?V…½ÜQtœ?IÎ9XÍéŽ?Eù¦×ÇèÄ?^x¤àTS?QÿýM^‡¿?ï݁ð|÷š?prÅ3?6f?C6:дѺ?M—­ÕqY?m°–7?kp*pI?ï……Ðäß?søòïpµ?_h¾ÜE"?Kï÷}d}?ŠÑš­cý‹?r³üé?Š2?ïÏ^ö83¬?S$6ª±Ðå?cjEk?Fþ~Éøgï?m6G]äA?LÊ¿ÁeC?ïÝ@bú(Ù?dH¿œ˜""?U–§{ùXn?K×Fß>âà?gôI€âý?b$æ@r«(?¥{$9?‡£ý'Ô?R'¢sØ?_K>'Ç?‡'Èui?…‰z.‹:?ïÿRÂ*î?ƒg|¼@?m^ÈB½~?g~aoߞz?št<¢N=?";ÔG
›?ó÷?q"W,)÷?y}9ð`­?dƒ¡î¦^?'Ô!@ž«ÿ?hÖU‡%²AGN4FGL J1624.9-4210?y»œ"@1ßv½À9°\'¹À;2{"¶
n@é¢[	;@,üœ?Џ½ei?äý®l@Zw¿á?þÌL&t3?ïê4†ðIª¿Þ{?[µˆc¿èß6üìOI¿ìxToÃÝ:¿ïÿþó…õ?è–ý]
wAGNbcuAT20G J162458-420657?Ñ(X‡;Ú?ÂlïmûJ?ÓSEˆ†ˆ?ÅÁqS2
?ۄŸò<&?ÆZŠlªù?ё4ĉ?Åi,vMº?ÑÛ[uǂ`?Ä!\þÖÊ?ܓp‡sô'?Ĭeí"`[?Þ¶)çôµ?´GªTûû|?Ä7Á©p?ª%uŒGl=?×.auC"?²pµè¸C[?Åä؀Îá>? ~Â6r#?ÖäÙ˅Fs?«[ÊOEÂÀ?Þ(¹ôHî?«ÎOv
b?ÀE34yž?´ÜìO°?Õu¼˜ƽ?Çäy=ûÛ{?á3Ô桵?ÈÂ`ža'?¸ŽÖ/µ?¼*Gny?ÚÞÌD¢Øn?ʽB¼Ï9ö?ߐ?V¤?È«¿‡¦
W?ÔA¯"z¬?²·H~v,?É-êçówd?°Mú!Ç?ß'ZûÉ¢?µ°Äõî2?£›Rà°V
?‰æIÛB?Û®×{b?µ!ů܂÷?àîßOlŠÿ?´}:*ÈÜMIXED4FGL J1625.2-3600?»"('Cµ@"|ڐî¢À9ô
 yóÀ;"Œ"ÎX¾@4ìƽ>@Ÿ¢È…?ÉQÄð_y?˛?áíEh@¤åýö;?ürµ"¡ã?ïþ{eÑëð¿Ú1/"‡•¿é³iï‡â¸¿çØ-Þµ'ƒ¿â¤C@Çp¿ïþ
ýŠúAGNbcuNVSS J162522-355452?ØÒMZ%æD?ÄÈÂLÒQØ?‡¢žâö?ˆ¼KQ5rk?ã8N×d¼~?Äõº4ˆ?åÖ¥+{·d?Å—ƒ-¶?«ÁÛÞáÂë?¤Gãí›fˆ?ÐÚz,õ_?ÂÀèE¬»?å"?D/ý?±Éš¤Ú¶?©¸.¼ù<?—¾ÍDfÃK?ÑÀ{ ŠN£?°O¢1q%Ø?å2V½.§¼?žÉ+š«?±Û-kP¹Š?ö[%:ƒ?Ñ$‡*΂&?šˆ\²óc?Ê5y°+gž?¿Úïû%%?'ô¾Óh–?'ƒ¨¾ ¨?èâû£W'?À0–ýUH?Õ§èÜø¾î?Çõ{pþ^¯?ˆ3lU?ÀÎ_…1ê?à‰þÊ(‹B?ÇÐصŽAÍ?ÝFUes]?²°­Ñ¯Á–?¸3ö!K?£`£R¡P?Ü´œ{©Í?³fV…¤˜q?֞öð⫱?¥c¤(ä†Å?Á-?H•E!?¢›ÂéŸ"?àe4µiXß?¦šøq¢MIXED4FGL J1625.7-2527?îÄ*©÷µ¯@0PÙÆ°SÀ7ÇϯÖÀ:ñq¤ˆ
%@JIOTQ@_3¡íûñ? :)­?Áªàú®‡@ n
ˆ~¿#@ —Œùù¿Ê"¸ç' ×¿áXß_vˆ¿äy`¿'F¿å(Ø0®µ¿éÜ°|¿é¹ÅÞñèeAGNfsrq3FGL J1625.7-2527PKS 1622-253?îí#'Lš?ÒT‰wÁ
?ÿt0?æÏÐé+?qpféÇÆ?k ïaÀÅô?ï¼Å#Ý0?…gî=ð,w?XD}$]Q?gdÙïƒ.Á?{ŒOtÒ?'®Yy€åè?íãEî‡î³?¤7Ã9öÒÍ? aɕ'Ž?œ/ä%³?¡iׄí­F?™â³¥»¤?ï¥Þ5wR"?pÀø'4¸?V›UcKŽ?Jö-Ãí?ƒµékYŽ?m"ºõO?îå6ïfD?²5£¥`?"Ñçtáö?±¾#cµÆœ?®!C¥$?ŠÎvVYº?ï?Ááâ2»?¡`–`W"?w«Î½wK9?–ç…¢]~?'ÐX"è?˜^=áÄ?íN>€³™?¥•¾a²Ê?¥Jj0›4l?ž#e=z?¥Ñ­ÃXk?œü\,\Dž?îðZ½Þé? Ôß0v?qp¡m@|Ê?d€AÑ(£?˜à'X­?ŽCUZÉ{êAGN4FGL J1625.7+4134¿ï¬ò'ØZ@F ±Ù+€À9Ê"
qÀ<qºnü7@‹#IWƒ@l¼Á¼ÎR?¶¨åf÷…Þ?ÄÍï»õå@êiæM§S@bÜʵ›¿ß¬;W¿ãÜâąֿæQ%AX¿çˤ® '¿ïÿ°7ßj¿Ð¸âÓõ5AGNfsrq3FGL J1625.9+41254C +41.32?ïà䃚 J?a·MŸö
?bÏ ÒÑ?[{ãžFÞ?X˜ø½&æ?M 6Mú?;dä?‡Gn¦QU?e}¿{ZL?t÷š­5—?¾LAÒ&a?}ËçR<ÁZ?è?{L\êY­?oö`í0;?tïˆè252?šIü{ À?pœŽ®ëx§?ï½ä©@?\9\ÇH?q‰±]Úå?R{uŸù?oå¹`¾ñ•?Qd0, Îh?烈–Þ©C?~2KÆkÎt?~íj½hIÎ?z÷;Gî?k…"pìA~?bÅåkö2?îØf EoÌ?¥émîû2×?w^Ó"ôf?Rºšwœ?Ÿ‡0e—l?£%Ìh/ª?ï9ÔøóÏÏ?ˆ†0´³
?R]ô"—w?€`O]¤¸"?ðÉeÀøN?§©&}`à?ï^¥°[Û?ƒBz`/Ëä?ŽIuŸ&fë?y;*%ªøÔ?‰Þá#?u¶ÊÐõÛ¢AGN4FGL J1626.0-2950¿ïÖ=LDYÕ@*§ïZ–N‹À7ö¿Ñ;ÇVÀ;O«›úœê@L;kæÙ@§"ÁÄO? æ……x3?Á<'§º™™@Øņ‡n@EŒê߇e¿È«]üµr¾¿ãS–JYÀf¿ç¥mB"º?¿èÀ;Yrb¿éüc'í"Ó¿áV[áþ`AGNFSRQ3FGL J1626.0-2951PKS B1622-297?ï¹2[XR?™Ê»šÐ=?g›‡¸ú¯?Š!™ŽÏ?w™3UŠ{?–CÐ@HP?ï©1<Á"ù?‡
r÷å9?^¡,'	p?kD´é?ß‹N{Û½?ƒ^as.>5?îÓ2يå?˜sÅÈÂ>8?‰•·Ú?'šŠ©ô?•~0T}þ?'â
´p ?ï®ìo²óæ?f†´ó8ݜ?a[œ¡Gv)?I7«5A.W?ÛùôÎ͜?cTn½³	n?ï±("HÌÍ?z¢ÿúA¿.?j8'4Cš²?o!èÙĽ?zOtÀÇßì?s(ª?ïF!2¼? UÃíÁi?qfp¶ò&?V–Ð<Ÿ?˜Å»?žOs/Íx?îb¦Lý¬
? Kv0€H?"†Øە?•;¤pã?žè¯ƒ9-?—`P…{ù?ï͞¡Ò?‡×XüLj‡?{ÀEµ"?kÆ؆‡t?–öK,kqR?"œH·ˆ$AGN4FGL J1626.3+3514?í±ïÎ{ðß@Eñ&|k‹iÀ:ý|ªu‰ðÀ<±vö×bR@!)æڕl?öÀ;ú'¾?Ð$þÝ@7~?ÐR9¦j@qŸÝ€y7?þ½ ŸrK¢?ïm­íät‰¿ëU.enâ¿Êj^¼#¿Ê'dÜx'a¿ÞŸxkK¨u¿á´¶á(#‹AGNbll3FGL J1626.1+3512RGB J1626+352?ïъx»~?f²gÛ®Tx?Nûú'úÖJ?B0¸<'µÔ?s[?æÒ¶á?d؂º9_?ïanٞ†?JK"Iê?n±àõe'»?r@bŸ3™?øDWú'?Š¿¡"?ï)ä‹8
'?†ZìDB?nêëa['V?l%9ý}ê?–æ+m·?…TB+Üm?í¿»mep?†'«ƒ‡ý?†¯!°Èî?hKYÝè?®X€ê^¼?"Ë B›ª?ï›9È+[?~£gÈÄ?_­öˆ‰@?T `K-ö"?…;ÏH«Ò?{ôÚÂ?îcœ3?§}l~–?¿µÔäüu?‹5Á'ì®ê?¥VRLG.?¤NŠìF~ƒ?5ÎæO?wI—áy%?tûâ_–H˜?q¤:De?¤÷@YZú?B'Ïiw?êYUÿ? ¨Ÿm"m?']ž®±?–ÂYó?îâSû2n? ;¹—ûY´AGN4FGL J1626.4+1820¿ï'd«Ÿ…@DãC0×8À:Œ"¦£mÀ<H'sg@u–Eý`@ÞûB0&?ÂhÁ_†M?ÏáÕ§?ÔM¬[==@ôB‡¿å;¹^Û؃¿Õ~àEO•j¿ì
c›°Ë¿áš«n®4¿à†FÁ—"¿èP%1€¬AGNbcu87GB 162358.1+182615?ï¸óõì¼è?€¿›—èÂá?k}fƒ¿?{mbÈh¹?uùF`ãà?oçBƃo|?ïʕ¹Ôç<?s°<î?Mÿr•ö?R­ÓêèŽ?w7Úò0?pnvGˆik?ï&ap³Fi?‰(â®R½?sø|F®*l?v'¿ò%!O?–5²×g·H?†büÆÜë?ï°å$©Ïê?a¥Fû®ãá?Z'môÐò?@+~ËÀ?€ti4Õ%]?`Iq`Ð?ï+L¤?Ý2?¶őó?äªX‰Ñ?¶•õeÁQ¤?ƒc'I†‡Ê?}HÂÉ4-+?ïUCÆÔ:T?'èg·5¿?a\k&CÕ?p±[4Šg?"5{ŸÏî?Ã mâb?îaÏåtÓ*?•ÈiS"´?†Ç0xR¦?…˜ËU×î?¤15‡?\´?'"º†!t?îÿxÊÛË?Ã"¬‡jh?w•yë#³?f"´ù…L?š*²oÏ&á?Ìq‰åY|AGN4FGL J1626.6-7639?ïÁ±7'_áÀ2͇+À:Ba¤`À<Rmý3œå@ /ù€_
ý@LÓi©?·b>
¬»à?^ê8§în? ˜‡Üéá—@	xš¶O1ì?×»©äÀ^¿ÊDAùI­¿ãqøjà¿ßŽÞ	àÿ¿àúÓOÍ¿Þž6œLÒAGNbll3FGL J1626.4-7640PKS 1619-765?ïöÂ"¾Š¯?EÅÙΝôQ?%RÎ2@W©??˃–F?O¢Á©¦?CGª%0ñ?ï랿ÑÅ8?h6Ì/B»?,oßúÃ?:&Œm~=é?b f1¥þ?fË4­¾?ï¸_æM/?q'‹ú:"_?MÃû+dVV?5íûy^b?€ÆÇ¢?púɱŒò?ïÀ¯§;Ýk?^—XR¥µ?RgHÀ	"1?2ê3µ´{?{ZH¼Uˆ?]8"ëî<?ïñä—Ljð?T˵?3鿲
^‹?-	*p²zb?W<aòƬ?Q7Ãâ¨ã?ï¿Îðq[?ò6ÉTÅ??~£[æ?Rœ>çŸÞ?~ w©=©?€ä"¨Éì?fˆ0w?FÝ]¶c?T¨a©*j¿?JA³tÖº?Œ%^øù?~hòöÂÀ‹?ïWF´fÇ?w\•èHw?h9›åË·©?QR"Šå
ñ?'µP¶$?w*Yœ0Ô0AGN4FGL J1626.8+4337?ë¤y('L˜@EÿO?Ù3ãÀ:ÏÀXJCñÀ<Š¬®IT@ÀjS†@g@€ù?ÈQ:€Y'?²²"Ç!è?ã±2!»;«@îOá¿£?ï¿}X›M¿êB€x`cî¿ê×¹Z)AB¿à£Ò¢Ï£A¿ïþQ€ž¡¿Ï•½ÁìôàAGNfsrqMG4 J162551+4346?ïȬÎn|N?…T*]g2?v(ÒÛ§Tœ?"¿Óø·¢ž?V8¸!ª?Pø"ù7>$?ï¢ÇF¿ÆÄ?…LÚË©f_?cœrÉ?‰a?q<¸²Ùo"?'g«$æ§?}²TLo±Ÿ?ïVt³Ü?~ö^
^=!?n4š«+V4?j·ýzF?'jÖ2ˆ/½?{Txqè?ïÅžƒý?\"Iݍôÿ?n%üý`Ð:?Sʘb2ŠL?lÔdµ#\?Púƒ?旅ؚ¾æ?ŠñC	ü?'ÏéTÊ_?‰†²¢"BÓ?\yúóë?\cî\uì?îïÃñ@?œÐŽÌ»f?u™ÿ"Ñ	?É'ÝŸ!S?œ¡òèM-?—ÑOK>X0?î–É¥Ð߁?'‡S%Ü?|_4âkŠµ?wò´R§ ?£	Ò:?n‡(Eþ?ï+¢J¹N?'³Öý?jÖ?Œ¦Û /ý?|¼,q5G?ˆp'¬s¨?rîÂW¶DÕAGN4FGL J1627.3+3148¿ÛK4æUxÇ@EŸå\ËOÀ;
ÿ'E7À<ªmà®+!@ ¨7F=Q?÷º›<1·?Ò×Î]›'–?Ò¹C£Bå®?ôJ…) z@ò‰§ß®¿å—O§Ýÿû¿ÝÔëŸuѓ¿äàNjDlA?¶g¡	$—¿à
¨à"Í¿å¹êqùA AGNbllNVSS J162712+314954?ïÏ`å6ê½?píä~u?R¡[ùÆ6?Kv<?¦±Ö?s§6cŠ.?ljóY¡F?ïÒîõõÍ?p²Ø}à?ByF'D–?Lœs~™PË?t9\/êH?mF¢TìÔõ?ï&²ñRæ?Žê²þÔã›?l Oên¶Q?p¯'/3æ?—•—×L­ƒ?ƒ.‹=<J?ïRR3·_?p±½,fÕh?_úù¥"ɨ?Jøœøë3Ö?"¶Ø%"'?pYõtÍ»—?ï¶Gh…‹¬?uI¤"'?YÆqŠ*O?LҎKÀo]?~j¯–ôU?sEÏ]™åÏ?ïlýgÛl´?Šf2Õcuû?Y-Ÿ³?aâ<ÀåŽ?ÍzG?ˆiï{,Ú?îŸÊwKÕ°?"6¿ÄKø?rHb•JÑ?r¦'ÉÉf¬?£ºV€ÿ¿Ÿ?"6%­˜çÞ?îC‡ò'‹?ŒƒÒ	&ä?mÂí‹[?auþÑÎ]?©ëYgª?Œk*ĚfAGN4FGL J1627.3+4758?æ,nÿ£J@EƤ~Ïé¸À:вýî­ÈÀ<™M߆ã´@Ÿ…@ò
¤@Ú`üšò?Ê0HÔÛd?ÏYÌ9©ïÓ@¿<pɖ·@"¹D8¿¿å塄õs¿àÝ6aé¿æbEÚÕ¤¿ëd¯­Uk¿ïð¨ÿ¾Ç¿é	lLþAGNbcuMG4 J162750+4802?ï˜g}<Á§?Ž•'ÃDÅ?sº;·{?€#RîÎû?€\C"-†?€³NK'z–?îñIÆónø?–ïÃΟ«o?†ßY.~õR?‡&½yµ³?–gˆšØY?‹V¦"ÑI?ï!¡²º?‰‡;¥a?9ç:âÙ?|Œ¸qã«?–~Ø'gÛ®?'¶ü-ËW?î°¿¯œª	?~g†"s)?–Ì`c•?voŠMr¢?"©~¾÷Í?rã¹#ÕÎ¥?ï°åx?ŽÛ&°?'ušëºü?x½†éR¼S?"ï/ѓ€Ý?Š×Þ¸W?ìúL'˜?µø¸áNL? †O›æÔJ?£Û4ÓÑV?³­v^.ž?±$‰
ûè‹?í°B—̇O?›–þM'?"þ"ôæ`6?ˆî½á˜#?ª|ÅŒ÷?"òø¤yÃý?ì.;ÐnJ"?.Väð}?¯fσ—?—'šˆ2è*?®ÜøKÓ)?'Äér´xAGN4FGL J1627.4-3301?ßßÃDʊ@%ëßm¹@ÿÀ9ÎÌ¿`ÓÀ;Ž1á#›æ@÷âzÞîb@BVÃ[?Ä¿4žBJÓ?Æ«:ÖÀ–‰@ÒÌ:֕£?öÙ6Âß¹?á¡èˆ6?ïüÀآĿê´k¬÷Dp¿âi`Kš2F¿ð?ïÝüÀ/…AGNbcu1RXS J162725.1-330322?å`ØKÊÈ?ÆGÎÞÌ?¦J'†–*Ñ?¥÷0×,?Òýì̞Õ?Å¢fkw{?äàšã#Xþ?Ì2?Ê]ٌ£½?ÅláØfx? …œ¹È?¿pΉ»U+?äœv?™ÀR?±*'oèbƒ?³»Žêߟr?¡øk»SÂd?ÑØ/Æ0_?¯F¯þ-þ?ãÔ'ˆ[·?°sI#ˆK?Ç6k¹ƒç"?§íÙ8 ?ÉyŠZª?¤¨9Ä!?ß±7ý6?È¥Ö4×Î?Á W	7rn?¼ø4ÉO-©?×¾¾yhÔ?ÉÕÇǪ?Ù/Ä4?ÎOê£øBF?ØF»HÉ{?ÍR€Ãg¦?ÍmH5u?Åá…V¶K?ß,!JlN¢?²r‰Œë'3?ÂK¤Mª?©B¼®•«Ù?×Ñ8äškH?°çun¼Ø*?ÔÁ æ·Q?³»]	?Õâ±Fo·.?·Dœ¬Ç¿?Õ[­ÒØ÷Ë?³o"u¡pMIXED4FGL J1627.7+0251?Ðötª»š@@{ñA [ÀÀ:" ‰ƒœÀ<o§yV-3@F‡"^qO?ýŽö¨hi?Îs€?ÖY¾?Ò"¿µî?ÿäùdŒW@	âe£û
¿å	%B°¿æ…ZýýqZ¿Ó77dENê¿á­š'w¾þ¿äÞ><ü‹¿ïìüLíAGNbcu3FGL J1628.1+0254CLASS J1627+0251?ïíD3[?QÛ0µÐìø?7ê·Ô®"?+§áXÆWª?_Þ÷à+"?O+¡TƶÜ?ïٍÁZd?o\±"»qÌ?D~¸IÚ£?MÑm†ȟ?p©HUߦˆ?iÔT«}òŸ?ïa#
¡(Y?‡÷Jµìò˜?s›Ýµu2?{'cT5#à?éMÿÝ-?'ó`–·÷²?ï{·ÈÚ?fP"??^îü˜í?=p\jéî?4z»E‰?dø²§á?ïלu'Zž?d®s^ßõ?G@AEÿR?9À25þÌ3?qI½`5±P?cƒ­£*?ïŠãúšn?"­r½­b3?YPŽÓŒî\?`£Ýãö!?Š&™LÅ?'£ßM?î¾ñÀ!BÆ?–…#´ÈÇ?'†bÍX"?±Wã&? +ó.þs£?'Kr\Me?îºÔ˜d?ƒdÏ.D?¯?k<²î[–?Vuß%Ïþ?¢žóTً?'xQ9ŸYAGN4FGL J1628.3-3343?é0Η'Ny@$±·|¯ÞÀ:ê#èùÀ;âo¼h@ Y¶Âs@Õþ¤¶-N?¾«>‡¥%i?';|¾þ"+?ÖÊû>ÊÁ@.d,$v?ïþÙú²¹%¿ëb†÷¿â‡k>gnÏ¿Þ1œDÄ«¿áP·b­IO¿ÓW<½J£½AGNbcu3FGL J1628.1-3344NVSS J162819-334342?ìÑ»
Ïß?²†d™UÓ¦?kàÄæûRk?}ï¯ßðÛ?¸"!ƒC?²Wu^d…?é˜`ÁrÉ?À%q–<º=?€hÜ·¢?…è^y¢?Ȗ½¼}c?¿Eª{‹‰?íp&{[u?ŸìV ¹?ƒAWÐÀT? Ýøo›?²¡FhŒ?œÇ½u%x?íÜ	Gɺ–?ƒ>‰á<[Ö?y¿#^"eÅ?WeGëA¦?¯‡Ôë?'±àX>?éÃäþ
Ì&?À(ŠÔ–?€[h`?sór~¦¼Ö?Ç굆ñ1—?ÀÂ<rn?âÅþ¸"k?Ȓ‰åœ|x?†´Èê­?"‡4è%ý?Ù¾\Gººã?È2>©çx'?é°Øø[?¯™RžƒD?–<O°z-?Œršï]…?Æy¹»Î?­â׌TÍ?éá#ؑ?à²¹Í­?'Â	<y4?w§µ×?Æ8x]pÚ?˜õ7'«ÊAGN4FGL J1628.6+7706¿î#Пó®l@A
[–(ËÑÀ9¤š~›çÀ<,žZÉz2@H¼áGX.?ÿS‡œAÇ?¬ß¾¥Ð?·mÅÖ8†Y@
Ý®ˆ*Ü@…í
´ôi?ãþC›`C¿×û=j¿à8@¹-³—¿á­ýžü¯é¿ä"q`¿åò"šCäAGNbll3FGL J1628.2+77036C B163030.4+771303?ïÌë™IEL?­ƒH•ã/#?Q Ÿ1/	D?"<ôR!àÐ?uB•@ã°?¨yYяç?ïä0n\Ôí?lâÊô°Ä?>RŠÑ˜
—?Kb¹ns±?h@Pdã?h<kd»?ï¸1:ƶ™?uѾÚw?\iÐŠ¢?Ui;6fa?|͝ãœÇ?u%/ÔÌÓ?ïî…¥½È?@GÉ*¬â?1ñï"\W?éêR"X?^yg>Åv?>Q{ÁI?ïë¶Ö¸?poÏN¼æx?;?êõ#?DåViæø?aŸ]Hº?l(®M?ﯞå«?"M‹úû®j?RÌ;½{b*?cÒZ©7}
?ßó'€Ã?'sƒþM]Œ?ï|Cf â¨?'O㑎?oHvB§Çf?r¢ûòÇ?‰Å
 .?}œ¥¯%î¹?ïԍi›¶?`mz2rWY?EM²,k2?2Ñ¢a]\s?sTÌxÀ»?^Õú2·"zAGN4FGL J1628.8-6149?ãÖßȼÀ"a'ÚÀ9Z귙^áÀ;³ÙésÍ@Ÿ¸7"kÝ@Æ[ê¡õ?µ›ƒ~¥!?Ϫw¢Î́@"ƃÝ@ã&q÷?Íî´(;2†¿ãf…·æ¿é|¢èÍ´¿èÝíPÐÒì¿ì̦×o½þ¿ïý9Fr«AGNfsrq2FGL J1629.6-6141LQAC 247-061?íÕW›®ƒ?Æ""Í_?¬>PB™ ?ÆTúG9»?Šy0Ñ*ÀÎ?ƒÊh>¶?í)½ûV?²lú¶1X?s³Çc†?zÊ&­ò¢?µ…\+(¸?±ˆ=7Ú<?î|Ù8¯¸¯?˜˜@Aþ@ý?" ~Í%è;?V±[¤?DZšÏî?''O'Å?îµÊÚ%È3?~ùý‡ ?Š³ýðqœÄ?j'œ;XEd?›ì¥Ã+>?y…þý¹Š?ìDÌ"á_	?Åè¼[TSX?µ+[éÚ?ÆGEu^ƒ?¡}=}¾¼?™òÂöL\?êØ.L;?Ä_FÓ_IM?Ž%»qÒ?™¼!¿ÿp?ÅÎC˜8Ï?Ã}	øÉ¢B?í
ßm¢"?¥áKÑ>&?¤g}vO?œ4ë°lã¼?ªº‹´WÆ?œmÍñŒ‹?맖V|Ý?›æ'ð<œ?©@›0à'?Ž5nÁØÂ?¶"ÿ³Ø?—<LÑ-ÉAGN4FGL J1630.6+8234¿írUB°1i@?:kÆ!·áÀ9
¸ª*À<&VÁ­´Ú@Îæcæ"@²>¬
:?¥ž»AŠ?¶Ì`@\'{@%äêÐÄ?ýTâƒBj¿±yƒÿæ¿ß^謿ä¥/š!~Ö¿æB• Ž¿êÛíÒt¿ç
'Kº"AGNrdg3FGL J1630.6+8232NGC 6251?èс'Sé¦?¿ä™9Cæ?ª|mu	¨‡?¡z÷î¾®	?ÆÞ]mïG?¼—_¶&¡?áHr™"Tû?ÐSÄh$V¡?֝ô/šÕâ?ÎGž©g±¯?»Dšp¦}¥?³â'é[?çˆk±s?±*þK•?¼nrÏUh<?¥šW'ƒÂå?Åb¤ê†?¬‰oœCbÃ?éi§t´Ä?¥Ú‹¾nøø?Ã،ÃÐ?£•¤70v?°š¸¦Å¿?‹qVY}ö?ßjì4á?Æ÷ú±rº?¹#‹Ÿx.?²ª?v!??ÚM!ÈôóT?ź°'5Ç/?Ö³ªD•8ê?Ϥ§61·ª?ߏ].æG?Ðß¾¸HAž?ÃyñNƒ?ºJ^'u?äOÜÊi?³‰AëYk?äni•?©ld>Ôt?Ë!Qgx?±`OÒÏf?⠟kPí?µÚF­Åg×?ÓÀùk!?µÍÙm?¾¼¿Ìî?Ÿ	BE‹)³MIXED4FGL J1630.7+5221?Òd‹?Ž¶<@E2\'ÑN<À96Jbú¡À<Ãõ¶7@G¶¶_øä?ÿ%"Ùîô??¨ø%
?Ž?¯Tkì @Oäë8@	l,¨T¿ÔzÁWÁ¿ÞÚÙÕÊ¿á*p·"@¿Þµ6˅…¿áÝù ?{¿æO6WªâAGNbll3FGL J1630.7+5222TXS 1629+524?ïæ|Áû=?lÆ'vgï?@óóõ)^S?Fßÿ¡¨ ©?eFAýÜ?h¯ÔwÃÏ?ïÀ
{‹)?x´h
{?T×28,ÞX?[¬J¤P›;?zÃu Â?t™:ƒq˜?ïµ|¬?whfùå°Þ?Wj˜€%b?\çi(¶?e›Çè}«?vIDáÁ."?ïluƒ(­¸?hÍm%±67?q"£ðèd?Mtã æT9?Œ•UÅ·ã?e?(ä?¥?ïÇrˆ'<1?sØYaþž?N
¶WiJ?EoUþLß?x…dö}4?r.òâ+Gó?ï6³"7˜Ú?˜|¢à6®_?iœ‹ýQâd?r¶‡dX‡:?•õýü"Xx?–¡Õq;K?ïqÜ*'?ƒ¨6Ô`?bù´}û?aìÐq˵þ?‹¹åC°Ñ?ƒ	©úb?îÂH "ïó?'ym½
`=?'›—ÒmkU?gÃÓ|Ý×Ò?ži 	rµù?€O.6—<AGN4FGL J1631.0-5302?ëª[™êÞÀ	ú D®…ºÀ9›)"N>À;3+­,ô@
fÑ@OÙâ_I?ÉÏìçÊT"?Ç¡¼}Ê0:?ÿÃ¥¦î?þ,iˆïú?ï—c"$ӿ犻°DÖÊ¿æÄS­úпëoÖ½—'¿É¥ì8Lø¿ïÿxáh:QAGNbcuPMN J1631-5256?ß:Ôè$A(?Ãb'n•?††ØӔ‡Ï?}xd]R6ž?àz(vQý?ÃTiNM?ú?äOiÙ§?Ž?ÃMÖ½š?ŠàŽo"?ŽAÝÝû¥&?֊'Ü=??Š"VÎ*?äÄuœW?°`~%¤ô#?¤-ßùY°'?"zÍ<
–N?ÓñYÝI¥C?¯Óéž*':?å'ä{6¤y?­âWè8'?'q.Oûi8?{pÛ¤(Ú?ÓÓ$$wƒš?­(™DgÁŽ?Ƕ³êÂoë?ºånÍEÌ?Âæ"Ö¯?ˆ¬3>?éŒ;ÐÄ0Ð?»v™~/Ÿš?ԫ͖ÔËÒ?Ãà0aœ¨?–âSlš¥6?¡˜Û‡ê^r?ä󙉝?ÿ¹šQ5¹?ÙIgüØG?³HGè›>?°¾\ï?šy¼éܦT?áX*‰ŸD?´VòÚ¯aÎ?ØòÝ¥§?³Ò§hãd?¡hÍdpn²?'ô2¦Í2?âÞy»ô!?´K4nJ.MIXED4FGL J1631.2+4926?ÝÓû8€@E`GýœÀ;$›À»GÀ<¨a¦
Ec@O+†®@ëU¹oø¶?ÉÀˆÊ>}?¿à¤ø?òéÆؗ?øµñ–°±
?ï*u¿á+3Šq¿í'ÿò> ¿Ç×ϊAaõ¿ïî¡UЗ¿ê;+ðHÒØAGNfsrqTXS 1629+495?ï–ÅúN?ƒƒ~ƒkH?f-¸l
x?e!`'RÕ?"ÃJÚÿ}?Äx?)Õ?Igkä?£‹ú…ÓÐ?'(flÑ?že"Y,´?™*Np²?ŽÁ¼\îí?îib ߪ?š~¦9•A?ƒ-«b"'?ƒý×µtȪ?¤žk$6!A?–Ürèô?î.¥$<J^?‹#+ÄU?¡k§¨Vôú?†h½å›~5?—T$Y.M?x"sé¢??ï"ž	¸2?".žÀ¹¶?ÝÆ0›?~8A‡®8y?"´üÚ-Hé?ìè;¢-?섒ó{üê?¶4#W?¤K=	-¢¼?«îð6(?±µÉàÓ!Í?¨æ0
ªk?ín%5ÏÕ?¡j%ÿD?<>=¶'?žxY½g?°Æƹ½o?ž"ب‰\Ç?ê[öû–Ü?ª§÷û*¬r?¼¥CÓ¶ÃC?ª~Úé'Ú?°{NH\?•V[.äiØAGN4FGL J1631.2+1046?ÌU®÷éu@Aü¸{Üð0À9ÌöÕ´ÒÛÀ<&ç­"ãZ@0&îV_]@->" 
Q?¹ñ:j_k?Á!Í°!›@^¡£SW@ÿ³ÿÌT?ïýZž²O¿à‰xïÕæQ¿çYߥ¥^¿â-¸j?8û¿í;‰]â3f¿Õ:Ûs-ÊAGNbcu3FGL J1630.8+1047MG1 J163119+1051?ïɼªžWL?rEõßÀòZ?ZNÂóÝÃ?`÷,Ÿ‹?tŽ%w:}?kDðÜâ®?ï¨p¼š?· ¸é2b?eaÇiºE?mu_=L?€¹æªPß?xŠY4wŸ?Øee?|5âòÆ?n+áE:Á?u4,«xJ?€Œ'4ß+?pûåéÿ7®?ïIm1å2þ?kܡ҈X–?"y¿%›£;?a;›æ;ºì?‰*ôiV­L?aß¿ŠCa;?îp-?ÑåV®¨?rÉ
ãµø?pÐw[ї?'Íܪí?våJ¿Y(?ïŒõ"·Ð?˜£ã¤ž"%?yW˜ØÕtá?Ð3~ó~$?—Ø{HuÛ?"'{Ã;?ïCÆOx?‰RYèIm?|¹Wl¨ë¶?XJúd2?Xà;Ëzk?"±Ø˜£?íÕ>auÌò?Š¯+†~zS? ]d'](T?'Â…pIÈ?¢Nµc²S?gümIAGN4FGL J1632.2+0854?êó·K–@AuT\x¦ÛÀ:7,ÅÇÀ<Eq±ôr@qjKÎ4¬@*"³‰.è?ºæPA
$?"'CoÏ?Ûå'`À48@
X!þ­o¿¾63Úg?¿è(ÝnÛî¿ä+3Šq¿ãg&f¿R¿éïm«Õ€?Œò"‡$çAGNbcuNVSS J163211+085608?ïè
8³áÖ?WítâÒ1?K0â7Š?;.ñÜj¤ø?a+{;²%?SÇtM Æ|?ïà'GHq'?lp ý•/e?A°ۇ?JÌ^ÍX[?k•?c‹t?g…"§¿^?ï®îJJüÓ?u†ó¡Åo?[Ë÷ŠD¢Ö?ag-l¼ð ?€Êîƒ/d½?qæmk–¨?ïÇ=9O	±?V«A'H?U†N¬–?7?ÿ"9ž?w!Èy h?TdI§Ó	?ïÇ
º‡ê‰?lþÒ6Ib?bŸÆé
Ö?R'.è'G?syÒÅXeý?g"éšx'¿?ï—ÏÌJ_¹?†½nîœÁœ?U§ýÁ?aYôŒÃs?‡W,R<ˆ?"zèÙUñ?ïZʱ"?"ÏX°"?k]Ìwty?o~ «<øc?';S[}Ç?ÿÝ¿eŒ?ïXbý·b?v[*o«Ž®?nÁí¡´ÀD?W½à+"zk?'#õéÖ¼È?t*… ¦ÇAGN4FGL J1632.4+5800?ï!÷Ø@Dzl <K
À;Ҙö«;À=µ?è@ Æ*ÚI7,?ýPaâs'??ÑEZ}$
?±‰Ä6Š?âi¿aTXÈ@Hñ0.q¿æ7­wa¿î-Ƭø/¿ÃÚÓÍ$á¿ã@9¿Ü0Ý£3Ì5?"gâèB3AGNbcu1RXS J163213.2+580109?ï髶Q¶?XÛt²
ì˜?(üDPÙ§	?åaÓE"¸?ekÜ[ª?W÷Sm?:?ïÀ!$µ8~?PHáQu?K·ü	W†W?RËÎ\qT?|xn;ì?}"u%¾üæ?ï(è"8^k?‹ª—‡Šg;?f'8br¿ÿ?qãÑZ¬ó?˜¨p™g'?‹9ºìŸ?ï×½Ñ(Éo?Yêè{‡ë[?3§Ä&Ø01? 
'kâ"?ræ›!{r4?YÛQ¤ ?ïÐ6Òá%?oŒôµi?4ïoj{È?(OOÛ ?v•Ÿ¢'̱?nkJdÉÌq?ïJ~þ°*?•xÚLá0ç?XÔifZƒØ?cJ
¬«–?•"ٖ+Gy?"!ƒxéø?î`Ü¿>?"!øóþ1?p5ƒD˜‹R?vªElº?§ëƒ©Îò?"õfg#a?ïwÐô¤­?y¿óåÞHM?F+×ÓÿŒi?=É'̸Š¿?T'²N%»?y'jÆà^+AGN4FGL J1632.8-1048?㣃‡«Ó@8Mqâ›k+À9Ï0âöÚ½À;ÆQ°Ì¼@),P•ï–@Z䢬gÒ?ÂʌU¹E?Àɽ£ºò?úTâ_ܪ@"šÞ=7™?ﯷjdù¿âº¾ý×0Ô¿è';2ô¿å¶<'gN¿îŸ™Þb÷F¿ïö±½|ͱAGNbcuTXS 1630-107?ïê…>*ý?Zö•{H°??³P"(9è?4ÈFP9?a"W?dk?Yâ
e&l?ïå~b©?iíàÞq£Ó?>&WÏîô?K>é˜ýÅ?f¼ÒCÝ7?e»¥|¶ž?ïWÃ^A²[?‡öDvnÊ£?r½Î¾§¸œ?uEµWúW?X ‹7lƒ?"µlê×'X?ïÛȏóŸí?Q™{ £ç?C40?*šk?þÆ?oS­ìÍ?PX¸O Ë	?ïÛèûùØk?€2& ­$?G±Iù{?BÅb³*­A?n*±'(x?í|¹u•?ï±+JþÎI?€ØK¼²Ž?TÖxց/®?búkÄÞ¼š?^¦1Û?}l._·?îß'WTG!?'Z$€ì?†y0(Íæ?†ÓH¡``´?™؀ÒPÚ?Œ"UâàŠo?ïšVv•nÎ?q՞åÙB?[Ö
:L÷9?IuÆ=¿?…ï¡L)·?oõ°çVxAGN4FGL J1633.8+0701¿æÆK×w~D@@Ú4üaÀ:>*ՖŸêÀ<QÑææT@<~"ÛH@½'Óh'?¿XÊ`OºÂ?¶ÿ¬ž6?÷vÙ˸З@	'øŒn7ì?ïŽ!ÛòÚ¿º½¿~/°È¿à©(ü¯i¿ánÄÙ¹D¿ä÷K[H%3¿êÇ/~ó¦AGNbcuNVSS J163350+065705?ïò1|¾†R?BûZþ×ÕR?4ÖßE?!ª¹¸Ñ'?VgôâŽ?@æ;ÄyÌû?ïÕ(ôÉs°?sGvçàõß?K)&/ŸPŠ?UFºŠ+Z?r`ó±ý6?n4>‰E>?ïƗêþø)?c(-¹mÀ?QûH'
??ô£"v'?x5I$Ā?a±Ï"Ãöy?ïSiœ%æ?iÊe¡gìÀ?tYŸÈK¢…?P:ï?‰
Ôe	©?g–Që¤4?ïçã¤)Àn?Qó‹ÌÖ¶?DÈiÛٔ?4ÃÕ3£ó?c©¸|/?N¼H]?ˆ«
?‡ÜÓ±ì—[?Z˜T§"?cÐÙzCã¼?ŠËô!ßՑ?"Ê•8V °?ìrb&?t˜ÜŽš±?Z1²/2·©?U§æ'1w?"R¤`W'?r–é‡^ÖÀ?î.f×Fñ?…ÆÎH1xò?Š(W£Z+¨?kãÈðQê·?¦"èÙ
?ƒ°F1)AGN4FGL J1634.9+1222¿ì…û'ñ@Aé4?¢­?À:øÓêÎ?"À<dInÞÛ@ #4ÔžÓ@(ã«5£?»­¢e6¿¸>Ú 
ëÀ@‰2"Ѽ?ûž"Ør}?ïûlb&¿è¢µ6®÷¿ã #Uož¿îû9Ç¡ê¡?âòc"úÎh¿ðAGNbcuNVSS J163502+122142?ï#"¶LqŒ?°ËП%…Ý?bJNøÖi?r®À5ÒWK?™Fy6›?°|&âAþþ?îõ
…q?ªù;¢ÙÊ?~F÷}Õä¾?†L'ÔÞÈ?™Ì't¤E.?©F»Þåi?íøÚ¼úqÌ?œ/×2ÇÍ?†Ûcày"?†á9½'?ª»{q´yú?˜TÉ?€qË?íâGÆ`?˜kA2?d'SsnÞl?aÌvFËnè?°K8x"…'?˜Õ»ä+?î®×¤Ÿº¤?ªÓêK®lI?wYÓm¹G?€Í¿9³úG?¢'KU`Q?¨ü'&Œ;?í¨Â.Á½?³vûLŽU?ÛÑ&š@?L2_X+?­|èËëWP?¯ùá
÷:?ìlB‹•ÊØ?¢:?O¢ßÑ?[,YKâ?ˆ³äeÉ9?¸²†þ?¡ ò6:e?çàlx'ý?·T/Ò›Æ?"¤oBq‡?Š'ðÜ5Eh?Ï4+öÜs?·2Z¼gŽAGN4FGL J1635.2+3808¿ÅbÃLNé@E*â:¸cÀ6K¯*ûVÀ;	ÇÿÞr@Ÿæè%@£$\֚¬?"}Y"M?ÀMfûŒ¨Å@4 uĨ;@!›fçÀ™¿ÉTå ig¿át·AË&"¿ælÐxR÷õ¿çP¼ R;¿ë·
è`Ý¿ïÿõïùAGNFSRQ3FGL J1635.2+38094C +38.41?îü,ï!`x?›O|9îUŒ?ŽßM	Î)?"£Ô£3_ú?'
ÖõO	ï?%Ægnv?åOèdÑ?ÖîpýL?ϼ激ø¨?Õr7;<?´³=ÌÂ¥?½1^ò©«5?ë¥:-'#G?¬Õ‰üñí?´䢜ò?¦AÂX"ÅZ?­xE_P_£?¢H°˜Å¦k?èӕ*¨?È02$ðF?Æ5g‰ÒÑ?Äp¾ª±U3?©ñ
"=9?¦1p@Äf?î§O{W?©€×Fq€*?š âeÊ»ú?¡¦ÝIÓ¥Ý?¡u(þӏ? TÇx<6C?áÐî î2ß?Ù\1›ÐÍÛ?×"i$9xÐ?Ù
=ËèvL?´îæf^«G?¼·3ïê?ì/bGGè?«¡Î™Ç
?¬âÇ«'ÏØ?¢epbª?°á²~U?¤9Ïó\~g?à\NßOõû?Ê]?ÔVY?Õ´'½
?ǘžjüV?Ã&v}F
?ºnÉvÖöòAGN4FGL J1635.6+3500?î–ˆB.N@Dü¼œÓà½À<¦-%ÒøÀ='ž>Dn@Õ³¦53@÷C˜Ü?Údò=I·"?ï*~ŸBP@.ðþÛ<Ò@Çy–™ßæ¿ïqÞ?ïýnŠø'¿Á‹½ãÐÊ]¿ãàâΖÑh¿ïÿx@XŠ±?å(@[9âzAGNbcuMG2 J163505+3458?í#ÿëvõÅ?²cÒˆˆ?£kýü…ý$?¤õË<·'ê?ªTIvñ˜?¦ÎÛXÛ:?êÕ¿ž!Në?¾²oå|WP?¹†_Fø½
?·WîqË?¯—GŒ‰û<?¥ÌíÛ ‰?ê§Å͐RY?«"Ëp§?·^ÏjÍ-?¦ˆÿXëH?³c&øq©?ž9Õ\êñä?íÈÝî¡ø?š¨"`ŒŽ—?´ÆÁhª3Q?˜mTÎ*É?‡×½8&¯d?z
77-"?ê£"¾?Àt7ŠZâO?¸Ááôª ù?¶­Ÿ='i?·)NFՕ?²çhëþv?äaÁˆöß?ÊMî \+z?Î]/²ÜG?njÙ]»[?Àá¬q§Q?±‰â¿UÕo?çg›‰w§?°¿jÞå?À"Á¬nn¯?¬|Û{néË?ÁŸç't1?¤D}ÎÛò?çŸèûŠ-?²‡Ï€{þc?ÌÒ9X?±~û'ç"?¥¯J&‡Ï?˜Íh-YãAGN4FGL J1635.6+3628¿åÅRó ~Ä@E"î9.À: á$r¦À<	t"&"@wæ£ãt"@ë&T' ?º0@åxjJ¿ªµèž~I¡?ënþ…¬|Ë@ªÖÍvì¿æM˜9GIk¿åcÉ2äXÛ¿æÞ£ßm¹A¿äõ'ÊIdοïÿö$´ë/?îï'Á8AGNfsrqMG3 J163554+3629?ïú§ÉKþ?G"åÙRþ?.3¡o›éÇ?'ûâ­¸™_?@`wÎý
?Ft‹öÎ?ïá]ꅴ#?r oÜ8Ôù?;—ÌÖ±n?N=³ÉTu?k/Ð+Ù"?pUÀÁ­à?ï€}V
ä?†Îàçû–(?i˜î`1ÏI?qԏþE?‰znèi@?"Ùôw¾'?ïöÛ	Œ¬Ý?:vÞÑâ^*?u`'rêb?ób+—&?P¢—!̺?9fСƒ²‰?ï÷jã"ώ?E£(teãd??®_b/Ý?8Š¸,»ª?B}-&_:??dÎ'uš?ïwßSÑÓ? ß¡£zÚ?L†Òµà)æ?Xú!—÷'?Þê.? ÇK #?ïƜ\¬?B`â=ÙG?xóûFi7?};KðÃEë?—ª-¬Ö.?‰›)O7*?ïÙÓ«Ž8½?a¸S&™K??ê^°	m
?2î]ÀñŠ?q"0œÅ?`gÜ(¬AGN4FGL J1636.3+7128¿ï|ÛÆí"@BbA=·ñÀ:ê‰Ê½fÀ<šlvJà@G`Ö@r$'–GÖ?»ÆUˎ‰¿¾4b2O2˜?ýûk{y"@•àZôi?ïøf–=ï¿ç_·ö{ó¿ëô(üxŒ¿á;Þ}yR|¿á@W¥ÙC¿ïÿèã«6AGNbcu7C 1636+7134?ï¼×¿Í"z?ŽH
øˊ+?pWcН?g:«[e½?q‡¬"Þš?{ßÄ®=¾?ïˆqT<S?Šd¬ M?l°ÒP[km?wŒ¢Â
œ©?†·vVüïˆ?§\:ìw¦?îÀJrêÙ'?"oqì›8?€ç2z5Ü?"N͔²!û?Ÿƒ`ºy?'þ\tœ ?A'ñ?ku;RPÙ±?pzZÿrîâ?\ŸË •ô?€Õ3≻?d-ßßÀ™µ?Ѡ'?0X"ÈÉ?€4':Ät?‰I苭
c?q‹jœHýø?qÖö—Ü‹?îâP¹ù,ô? róφj²?|ƒš-Xá?ˆ<È´ïs[?œ•7-7?™†d¸°Bû?íÿÝ­sk?™b3âì¯ý?7ǎì¹Ê?¨)'Äæ°?§æKÁ"c?"éË3=_?îeÕªåò?'¢Ã†I}?"^}q—]?†ÔÅIÌK?  ~֘Õ.?ˆ]óG­5$AGN4FGL J1636.5-0454?Ô_Àá:@:óúã`	À;"ˆ\ÙöÀ<XùD$?@!ñ¨Ôõæ?ü—ù1~'?Ó3®BÈý_?¨$ j»'?Ñ» |ø#@G6·!>ê¿å›¥"
ñÛ¿íàœ…˜?ÅYGŸœ¾¿æhãï(Ah¿ÑßÇ[Ýá¿Ï…òGۋ×AGNbcuNVSS J163631-045506?ï	-ü´?šÈ£nðÓ±?F¯®þE%m?=—3ӝ¯6?œ)\Ãðó,?š|êÅՆ?ïX4?U^	?•ÿsöÄXd?k(7Õ?r
Ou;qí?'"dl	jA?"º¼ò¿k?îÓô»B$¬?®
|¼Õc?c7ƒœþŽ?_Úð(×ò"?¡<'Ô?GûŽ£"»?íñu0?{Tž¸ž?TN¼Ýà«/?C¥LÀE?°#r)?^¸ã"÷?킿•wæ?°‰÷œüqø?YayW@?Q/­Öá"m?³"'üI<4?°méÇÂ<t?î¹På[ö?£{|Z7?sr/MB¤z?'›È¿í+j?¡ü«¾ˆ‡?¡Ÿ¸M[J?í%7Ú.V¢?¡zUL]ˆ?p¢wæúÌ?k£*Ž2V?µÌ¯Lµð?¡«­oÏ?éÖüåÞœ?«±a-ä·?býDäŒ?]›2Ãóž?È[ÈrõëÕ?«¯'=0LAGN4FGL J1636.7+2627¿Ðg™öÐp4@DŒÁDŽÀ:Q÷·\"@À<§".Î@âPÑQl@ÉuDO»)?¾i®oišM?¹
·ß»øû?ûŠYUëÒ?ùgÐáÚP?ïþ˜â9›'¿Þ†#3‹É¿ã<b0÷š¿âgpÛs¿á³´,ÂÖª¿ïëÿÝÆDHAGNbll3FGL J1636.7+2624NVSS J163651+262657?ïcݦô?‡_¤#D?WŠEOª·?J}Щá¥?'sÜ?†Ãixsìý?îžîž"ç>?˜f0Í?ŽpÎEß‰?‰ªO¤vû?œéÅ
ã-ç?ÃÇeèd?îÊíXÕÑ{?"%#ÇW?|$'à-¯?}	x3¡LÖ?Ÿ›ËÁí=?'–à¦ùr?ì²P{²AË?ŽÄ»}¼f?¨w‹y[»±?'ë'ÇÚªõ?¬clÎܜ?""›¶{èß?î³ç•ò×?—E䛞S?kR¢Ò‰?_ý P§=>?£nK­À}?–ˆB=Ä?ìLêñÈQ4?²eáÈfÉ~?¤hKc˜»)?¥'Š/Þï?³d'¾9JÊ?¦0}þLe?íß,ɕ=r? *. ÓÿÚ?‰xC¬©Ëÿ?†,­Uo±?«¯"xå?œ­ùàǤœ?çè±	ÖK.?¡Èý9›?¼ô¼YPíó?š€z\ê$?ÁâݩؚÐ?›£•ŒgٍAGN4FGL J1636.9-4103¿ìBlÚ|ki@€ÙÃUTÆÀ9zþ‡YûõÀ;)'o(¬Ç@{1ÊÓMo@Æۙj?ÈWÔþ©c?Ètè_Op×@òyÝ;¯Ù@ÊsѳçN?ïÿÖyô¸¤¿Ã¸«Ãã¿èùD$>û¿ä?˂þž¿ç|éàƒãпïúšï°AGNbcuPMN J1636-4101?ç&L¿e?Â/©®î2?ƒÀ½éeÏà?•—¤gw	V?Ñ`'‡ž½?Â]
XYÄ?ᶷ¼+r?ÂâW‰ºå?°aAã‡þ?ª,+|çyz?Øz@¸×Í\?À
˜Y*5?æ§Bî"n%?±ŒØNIßÔ?£Æó*?Õ¿?'_€ñ«?Ð8›¾s(þ?°JVòµQ¢?áá¦nqÖ:?¢šÑ
_uB?°
ÕÜCw?‡Š"'íYà?Ø:,­nHï?¡•Dój?Ø|´—²ö?Ä&Ü& Âr?•N@b˜<?9Ø÷z
ã?ãJÏ3PÜ´?Äk w¸?Ñ6ÉÉzL?Á"M@…?¾éùaE?½×üdÁ ?ã‡\IpÑ?Ã0è{æ§?Ú#‡ôց,?²ozBX˜‡?´¦—‡ZL´? æžœB(_?àYiiS?²êš‹X¤Œ?Ðf¥ÿŒ^?¢¾\ØÕa?½|O"³s?›Ï4Ïù#®?ä#
Äq?¥SÀ_jÄ{MIXED4FGL J1637.1+1316?Çóàυ†4@AÚ!xöŒÀ:úmPes!À<sÝo²?ƒ@SØæ
¶@u ÝD?Î4rÎSµŠ?¸"éclâ?îD½¿h¶"?üÛr<2‹C?ï³hëÒ¿áúóPÅr¿ä&Iàô¡þ¿Ö놡D]Ó¿êàˆ!ö¿ïÿý`éNäAGNbll3FGL J1637.1+13141RXS J163717.1+131418?îêé=¤Xî?¨ÝëxÌ?s´H}?y¥ÉÅ/ÆS?Ý‰'X?¥ *×iêÈ?ïF¯pÕ#?‹K•R|?wh†æ´`?s/©Á§ü?'OðE\\v?…_3ÓR^-?ïl×Ϋ?ŽËm7w Ú?wšYNM/|?wíºÈm?šåê¿¡Í?Šë4+Ý}?í«ê4øÁY?"Ÿ¥	Tâ?"ÍËÄFèÞ?qçì¸ "?ªÚvÐD?'KÄ>}Ó?î 	Þ?¢º±.p2?yü"š:+0?m)ß¡?ª¿ÛÊ,
Ä?¡Ñ8³ly?îý¿¢±Š?¢"d5ªŽ?ˆŒ;e?ˆ›""å?¨®*?Ÿ¥"áAÓÿ?îa%^ß4?™×­)'¯?ª`›1-y?yá.–g÷?ªU'SÜë?—"™GÞ<Á?êV±2'?žL×·¦?¨ª©@¾}?4(¶Že?ÁÝýXù–?›:‡!bAGN4FGL J1637.2+4327?å¡+§ß¾¨@E
ÆûÒsÖÀ;ÙPVY¨éÀ=y_gn¤@!'ïCš3?õA³(¶Ø?â`€É>"?Þ´Ù% £y?ý	µU·Âz?ìsö™Ïտߝf'Ú?ì8ŸÎz¿Ø"€ð«N?µÊ£QÔ3¿ÝÜ°Úþ¾·¿å95Á-sAGNbll1RXS J163711.1+432548?ïŽvœœ?'dhÍXj?lµo¶å»v?põ:-¾G?…P†iáÒ
?Ž|uÌ~Öò?ïêód¢R?™œµ¹¦?'Æo½?‰G‹œæ1 ?"ÿjµÚ3?bÉw"ŽZ?íÁ
ð}<? ýËVÜÙÖ?L»Û½õQ?ËnŽêC?¬/e½+í?ŸM§ãW¬?ìÉͱy4I?"MløÚOu?˜¾ïÈb?ˆ<vË/á?³Öƒ²Û?›¼îå#Ñ?ïg#±q/?÷ÑG ?~V8fè!?Šg´Y_?‡ÿå2?'íww
Þ$?íOõt€Ä?²ëd"ŝ˜?šØ¾Eì
?¦/›š—ô½?­"Iže£v?¥ŒFR<f?í—µ‹4?¥ˆ'¶*±Ë?Œî."v©?‰¡¼?ªß?´|"9Þ<?£ª±ßª?éÛSÊú²?ªýñˆÉÑ?š>ç$˜`?›#iv1Á?ÅJÓî$"?¨ÎCih!ÈAGN4FGL J1637.6+4548¿æ7£Eûóè@Dý\B 6À;©%ʔä(À<ùZ'ó+@!¯…>BÜ?þ¡YKË°m?Ëz©u¯°?OöìˆZÖ?«¾œ!M€@~3ˆ˜•c¿ïÿT•Ð·?ïÉL¯Ûû>¿ãÆ'+½óì¿éC•ìeïH?ÔÉJ àuK¿ÛÈ…3[!AGNbllB3 1635+458?ïÇ{ƒüEÙ?€1w¿§¼Ç?OÖ)}cZ?tmŽ•qþ?xIËZÛé?w¯"Âï"=?ïÎÖ¯{?v5÷FgªI?E´z"g/*?PN–
-=?uÞjÇj|?s'£'‹T?ïC€Þ6Ø?ŒÕñ*þp?dφ·Pûü?i[F½–>?œŸò~Š?‹÷±
9àˆ?ï×ÿ€~?¡?]Ï\UŠ°Ñ?1þÏâ¾#Â?'ÐPsr;Œ?ràRÌÖÑ?]œOwӞh?ï¡I˜¶?ÛéÝk5ò?JË%½ñM«?I;-dí?†{Kk\q?)Éj&@Z?ï~_&´¨F?Qm"¨Õ&?Qû4çWÛf?_‹¶i?Ž(ÏÃQlè?,ìb ?îeóOv‰?'=Yöø?o½_¯?p‰\52³?§¤õJ˜?'µâëì#Š?ïpf¬¸Z?®Q }VÌ?LXò6kR©?KD 'uW™?'`
Ò¶?‹º/|Ÿ'AGN4FGL J1637.7+4717¿Ø<Ý\x7/@DðÀƒn˜À8Þ©°â‹À<Aæh2ï@LtQ‹è@,Âþí±I?¢RFýHY?¬&|w"@¦#×þ@¹Ûÿð'¿ÂGpÂ_ág¿äv‹AèÜ¿æ8o'Á¿åM
švX¿è!£=Ý0G¿ëZA"õÆAGNfsrq3FGL J1637.7+47154C +47.44?ïö¢vb?GËËçëØ?$¿ûjÅv?
;AgC?P#
…¶T?G3HÁìz?ïÙaºÒpÈ?qǐºçŒ?B+Y3ëê•?QŒ?Qã?q	·Œ½Hæ?pr'z?ï´â»ªK?{çÎE?WïX."ŽÕ?eõ}Êuúl?'Ì#n??yõ桊(ã?ïýGŠÖ;? ²ºó˅?f­lh?ü©êu?-?º'`?˜Tnšþü?ïíÊ¥Í{ì?UÞÕіլ?.jó
ë¸æ? .fuå?`Nªå˼!?UŒ|?3¤?ï‹F €ò?°££&?WJB?nß1$?ŠEh)è?UO`è?ï~jÂICÉ?ƒÑ|AÁÅ?d*+:~ö'?m• µ•4?‹ZĒXÂ?'}ޛ_ü?ïøŒÊû ?@l¾®Q˜s?5àyª?)¢´ fƒF?C@	«›ƒ?9@Ý~$AGN4FGL J1637.7+7326?æ;èʕv@Aœa|ÚQÀ;»`iÍ#4À= á÷×=@ ÐåZ7Y?ú̓ÜÁ6—?Ñ&Ÿ|¶¨?ÌßI¼ŒÂ?ùñÅû!sî@g°'£#¿î@5¯å5y?ïÛù%k¼¿á2:DŸlA?Ää^ú6gp¿é–Š ØR<?—çCp˜AGNbll3FGL J1637.8+7325RX J1637.9+7326?ïÖpÑ>2?©?VêãÝ6?]uþb²®ê?"Z̞6ˆé?jÔè¾/§?ž/õ@RcL?ïæNº3~C?jAšu%â¹?<†
Þ²øè?HŒ–êX#æ?f "<À°?e"{׍?ïBæ"Íú
?Ïûr«?q֔_gÔ?y¦ë²X;Ý?"-–-%g?Š´dÞíYâ?ïêy~y¶-?G¯Üõi¤?D!ý"È?0x"k#?`…8×ÁB?D×ï_ÄQ^?ï¹Áם­?¤‡âa.z.?h%!_é¥?‹Ÿàjo?wƒŠ#Zÿ?›Š¹ >b?ﳚQÐ?€ìy¹H_?PÅo߁^?]"hÍÕÔ?'N%ºh3?}ð«
x|?î§[÷Ö"?–‡ßšËA?xW[=^Ìf?~…ÐêÒ)?¢U.]7?•Ã{âîZ?ïÇ5ÿÉ×Ø?eÏzè°®`?V™.'m8-?PòèM&?v¾´z(a´?b­CeŸ‡ëAGN4FGL J1637.8-3449?Øh…íaº'@ L׌CoÁÀ8ì=áâßÀ;²ïQ/@ h½1øv?ý"
¹&&Û?°?lÒf>Î?³a(c÷KQ@¹üȽ@ŠT©$¦þ?ïìæè×ÅN¿ã2´ˆ2i	¿ÜÀþè(¿ÕN]Ƅ´/¿à¾há?öe¿à2ö—¡qÕAGNbll3FGL J1637.6-3449NVSS J163750-344915?rܸË?š¾Çë*?Põà‰óX?C½QvËY?¤™Ð6"Ú?š_1¡Š?9?ë¸ö¤¸p?·6,cTF?x´Iÿk›0?}-áE¢
?ÀVƒë¾ç?¶†ä_ÎbG?îv"Ÿ?•ú§B2]?rÕj£ŠzÂ?tÍÿY;£?¦<"©¤ÞÚ?"Á½éo¢?ìòÇp"j?‰´ç'ú~ˆ?'Æ)¹oŸa?k»¦Ußñp?³¸:É»X?‡}ͽ?ìª6«u'?¯æÔ0ï?r3'	[Ä?›	$°¨BÄ?¹‹ˆNà¼?­«1S~½?ælo¾:?Æá Ûú‰–?ŽEy]™K1?u1‹¢½?Ò4ô¸gÿ²?ÆB­éK¢Z?ì͂«'?¤«1ûå9?€A6V(V?}
Ó¾=?·''Ê\J¨?£u·±‡?èâ^ËM¬í?¡M†zëÊ?¥õàþn@·?†H"¢=ar?Æù"-¼?Ÿ¯_
2–ÌAGN4FGL J1638.0+0042¿Ö¹3<îH@=¦ë¢zé«À;-¸éÀ<‰¿1×@"(Z)ÂC?úTœ×%?Ìvì…ú«W?©T"¢Í±
?àÖJ>ès@]/Ûæ¿é««Ÿ«y?ïÿY²"ý[¿èöÝÂhp?¯p
BèÌ¡¿ä
Cë[r¿Æ¨Ã
†AGNbcuNVSS J163809+004223?ï¼åíæÌ?†©Û=ûN›?6íUïì=?*Î
ùQD?€6=V?†xÝ/0æ?ïÍÊ«µP?t'¯Dþ™?J²—Ôf¶®?Tk¿n{š?uÄW.¤Q?q?)f àf?ï^#*Õ?ƒË}r>²S?Zí1O‡?E»,Á	|œ?'ŒÇ¥ÐÇt?ƒžôÜ
B?î¦:Oº±?'ƒQå@-7?t¤vÌ¢öß?`±uxñ?£=…M…?Æ°e§fn?ïŸK&fhŒ?'¦«Z؅?ESºè/x«?9äáAuLË?†×ú²¡?'`ꕴ*?ï^—"J"?'`'/û—Ò?`I'՞ºæ?jV3ù¯?'#èMe?§-)v?îçºTب?Œ
ˆŠF?banp¨4?XÄä¦Ö>¡? ho´eD?‹qɪf?ìc|•cU?Ä*©Ü8Ï?‰Chœ?~\˜æÐø?¹»®RŸpY?œ÷~HAGN4FGL J1638.1+5721?Ñ;
Õ=@D/ŽèÀ9Í|ÉV À<†ŸJ³'y@;Y:Æ@Ü6r?±¦îýàQJ?³
è³³ ?übÏØðÇ~@°ŠÖ2Q6?ÑÓ-äê¥Ñ¿çßÂ=&Ñü¿æôV2ì¿ë
`¬B"¿ãæò}`}ï¿ïÿ7J³AGNfsrq3FGL J1637.9+5719OS 562?ïø©P0h?=¡ò«ì>8?(m€eî?•¼èº?G?ye¡Êó?:
ðæ§Û?ïߕ%ãá´?nwm‡sÖ?A(Ô÷þ°{?I2(
Us?l ¥ý¿2?i°ÔL‰¢¬?ï±Ú:?xTµô¢"?cuE¹áû@?r9·-©Ë?}X?øäâ?pcMm¡7+?ïó眘ã?8"í|yúd?FF¸]ÐÝ?,¢úH·{?JÕêò M?14j[¨ª?ïÚ1	n"?§ßw=[ý˜?E¥Õ?wö+ìNg?p2ÀækÞ?¤áæó±Á?ï•{hðÉ?ˆ0<ÿQé´?Vv2kø?b5Ü`È?‡ÝcRG»ú?†d
ö¬§æ?ïu£¨'.;?5|Qâø?hðtóN®?sr³W¯	0?ŒZøÐß÷?|e¬	`4?ïØü,Ùa?]Å:M»?bÛÞ?Qé"DwS¡?d'ã™ûè¼?SRHï×l¥AGN4FGL J1639.2+4129¿îhg£Zì@D܁Ü
²pÀ:^þُRïÀ<HKv @õõ0Ä@ˆœä§´å?ÃDuû°?Ðìà=—æ@
ί%@8у?ïþ@bEÅ\¿Ý݅íjñ¿âÁ}
q؊¿é!¿îB¿ëK¿Ê߀ƒž¸AGNfsrq3FGL J1639.8+4125MG4 J163918+4127?ï'Zè{Kr?¾L'èíð?lļ2&å?gI½¤íàñ?ˆ8ÌêÉ?|YI…ú'B?ï³8Ž"(?'è`Q¬ù?Y%èùÿb?cý€€7W¹?€´°)»?'[3²}ùÒ?îܞµüëg?'ay<í?%òÄ2hk?ˆCWr̉?•Ù/×j&é?‰JSù5èC?ï˜Vj'<z?ce§qï?d`'ao·Ã?F³äa9£?"ÒD´N¡…?`ö@¶Ãé×?¯Áh?™á
wŒÔ?Ñ˜^ý?zʞ.1Ì@? ešà&×ì?–¨Ôq+h?ï,[ÈӘï?ŸkûW¢ôÏ?gŸï('J¢?u"¸¸É?—€‰ÿvÌ?œÉ¿†{T?íj±2×1™?¢%×VÈÌ~?Ÿš¾ík?")ÀM3F?©‡\ÝA2?›"]ÕXC?î¼q[¬=?…6-Ñ¡š?|#×DÒÇS?fô ŒæŠ? ´ofrÙD?'ãWç<K AGN4FGL J1640.2+0629¿Üü͟ÊO@@*Ã") À:º$§5jÀ<f®ITè@!P5©/8Ó?ý}<9Aj?¿Ž9ø¹¿r2byíŽ?´; C¦7@ùùü/æÍ¿èÈEßÞ"?êBÀh Ó¿åù#7<­/¿Þº/(¸¿ÖoïœZ" ¿Ô1"\p™EAGNbcuNVSS J164011+062827?ï¶LW=öÓ?†oc´!´?P4º¶ÃR…?Jö‰É+>Î?€fRΐ½™?"û¼f‡¥O?ïÊæÀË?t=8tڀ;?KCçòæÕ?QY˜÷*û?wŒ:$?qÂ,À¿V¤?ïqQ`tè?v¹(¸Ød‹?]ÓEÇëR¨?EŽ1Á÷?ñU¬Õ—"?uÉêƐ#J?îßÄk
"?{2Œ«²¾^?qVì*H—?V<ïê$î?Ÿ±ÄiÄ[?{¿üÂ"m?ïUîҎ¶?€>uId°?[ÔY¾ú/"?N:ïÖ}é?ˆoù+¸l?~JlkÖ@S?ïið äÑü? Ø¢úކ?]…÷ɃB?e^*P3:¿?éœzðB:?ŠÿŒ–«ò?îØ,²™""?Š²wâ»Q?f"ÏûbÝ?U»ìqW,?¡²¦ðj?‰¦Ìoö+B?ìËârŒ ž?•¼g3|?‡*œ
ž@?v™-Á4åN?¶»¨÷«SÉ?–ÕÀiѦAGN4FGL J1640.3+6850?ï¶oªÕ"©@BgNe¾ ºÀ:ÃfÓ'ºÀ<ō²Û‰ÿ@(j[i@PÒÆÒí?¹Ö°™†¿ %üCÕ9?åƒí€ ¡¶@š¥'Ÿz.?ï¦Eÿ¾'¡¿ãxK é'¿åMåр´¿á¬4Á
!¿ÜÈ+'¢"¿ÝmHmWpAGNbcuNVSS J164014+685231?ïø>s™?]â¨LTd?(ÃÀóN@[?&'C™õÖ?HÖý ?[ê9<B¡?ïç½ÿÝùÎ?ii~ï€H=?7j¼ó—1?D6ŒWû3?eT¨¬µ?e×­#Ú½¶?￳qÔ??k-Ò¡z?Q0oðü?TAw§ª÷	?{Ú3"Çk?i![w¦{é?ïéÿfcG‰?G¯ßô?BïÒݘî?#\H5ˆ.?aO­oí×<?GP‹Î.x'?ïò;èþš?Y·ÿYÀ§W?9¿sö:²?5V_¦bc¥?UQd‡x4?Uê~wuö†?ﱛG]{u?'ZY>ìï?KÄ~£Ò=?XëO1RÈ?ÜæL‡‡?€F"qa <?ï'~xr?€nߪ»!?Y¬}y¸àª?^zª½A¸?Œ*èû›[*?~¬;'?ï´ðò"RO?fŠ¥
׶5?^'Î#>?JŸZ[*?}âÓ7¼?fŒ°ÝÀAGN4FGL J1640.4+3945?ë¾7fÚ»´@D¶¸ºÇÀ8T¢eðõ¡À;r:?–îÄ@àðÎ^È@ ðÀÇÛÌ?§É·n–¶?®ùQ~ç€q@ÂÈ>Ȓ«@úÕOӿܤ–LÝÿ$¿æz8«B8Š¿åÜ7£Û<¿å3"6‹­H¿çþŒ}Qdw¿ï>ÎÝHEAGNFSRQ3FGL J1640.6+3945NRAO 512?ïîŽR‹	«?Sj`}
›#?1'çíÁ—?+Á?ûH`?^' Òr§?Qô×ҕ0Ð?ï×âæ\¶?n#iºwkb?F‰`oÂn?M¾&ð^ڕ?q=aF)ò?izlœz8o?ï)ŽP²—d?"ÇzK¢J*?ˆdƒ³?re`™j?Þ±†\?ˆa'xc?ïåô KÖ?Qø3ÍËÇ?B14!Üq?.Ջv@e?e˄ÜG?P]¸ÔU?ïÜn"0žÙ?eøäÿ…É?=}ÎÚ:•õ?1^­˜lè?oá³#"o¶?e6'³?ï…èŽcw?‰ø´ˆè"T?VŸ³òZÚÓ?bò=˘¿\?‹±åõûŠÉ?ˆ†öWIb×?îٜòr+t?˜çxZëÅ?Œ–Ôú5G?†"r?–€÷9ÇqÐ?'ËÄ`¸?ïºÓTj)X?oñ¯‹mŽÓ?\1~·œã?O—e¿¦äP?{‰öõ— ?lò¦{b
AGN4FGL J1640.9+1143¿ë÷/R¼@AJýTTÀ:%ïpeéÀ<?gÀÙyƒ@;‰³¢x@?Tú-X(?·(xD4b]¿DË*ؓ ü@'drñ9¿é¦Ž¼-ÿØWv¿$·¿èt­Q'Ñ¿ä0œJNì¿çâC5à?ª	CÜ´Ý~AGNbll3FGL J1640.9+1142TXS 1638+118?ê',×	ÍÅ?×=+Ç%U?`flšÑÊ?z9³jêÐ?ŵ²ð¾Õ¤?×G$P[&?ï©L£	?'l;,ÈÖ3?ZØõ"pS?a)ܦ–M¦?']èâÛÒ?€J¦?îçeB¶=?‡
µ`€'?~V9;Æb?€/°|ÌÀ?›}´]U º?‹~Û{†÷?ïYN‡Ê ?py5ƒJ?s§9®
3œ?V&*«?Øà÷êf?k;'|=Ãþ?í6ãi?ȶG"Ï?t '"Ã>?pãd Ì¬?µ
ç×çžd?ÈÔÂFƒiy?ïÿî•Òî?"0³5¨×›?mŠüÑTúa?s·^¾3Ò?˜î¢›²â?'ý˜b0"'?흂.:rd?ºEcÑ?.¹îý
?†ç5Ù«­?®\. ™–~?šOp;ãl2?î
‹›÷dG?țÈo†?ëÏ0$A?w¢d¦Ã,Ì?§PÐY͐g?‰‹¥´0ÓðAGN4FGL J1641.9-0621¿Æ¾Oj0~@9íÇïzÀ9'-åìXƒÀ;©pÑ#s£@
+¢F¨@68ù€Š?·EH´yĽ?ºþð¶`ú—@Wš»ØˆÃ@
ÉÂK"}ü?ïKøQÆ¿Õ}Þ€iG¿âÄßÎ1PÛ¿á߆®Š©¿êb…Ñe¸Á¿ïÿÿ" 5•AGNbll3FGL J1641.8-0619TXS 1639-062?ï×hRŠø}?bße¶Hâ?O—™Ý¬ÿ*?@kAH	s~?pXãk&Ãÿ?`àW" ?ï¯ÿÞ¶Èî?ƒ¦äeÝ?e4×&ZÆ?q(k€?ú?}wö0_?wóÐqm?îú0\¶†²?'µšiâ2?…rڝWÛ?†1 ©2?–/:ý˜KÛ?è3ƒ€?î\q‡ªÀ?~Vù¥·à?o[°êhö?ioÔúoԙ?¢ÝŸ‡Ç?wøjXèP?累ߺò?y
@Õ½:?d.eµè·ë?Uüï4lÍj?n˜Q)š?vï´ÈeJ?ï2¾•kPu?—zîŸ	¹ö?v:h()â?"ñöüý¨?"%^¾7å?,z4ä4?î"iýðÜ?–bZo
š{?[™¤nnO?‰a§c&ƒ?žås2M?''Њn?ëæë©SBj?—¢6ÖhÈe?£"4ýi ù?….Wx¯5°?·ˆ6C(·?'ø¿¸3°AGN4FGL J1642.3-8108¿ïÿÿô¹È0À6+¢±pPÀ:ŸØvN:öÀ<$iϘ@«FjGœw@âWãì¤?À<'ùn@z¿¬\[p¿?ëXm_)]@ã%Íïâ|?ᄅSK¯¿ãI€2Wk¿íeK´3xÓ¿ä¡ãÀ¿ ;ƒ'¬¿ç·fÔJoAGNbllPKS 1633-810?I{Z?›Ù=žqÉ?rû>ÓÓd?|õøòœùv?—ð®RÍÓ?™‹¶(±Õ?|›+?ˆ‰°›ÓU‰?`æoÝFæC?lf‹MD7-?"›"é#é–?"…O1Vê<?텍Ú.ñ?¢lÀFÒXo?‰XßFu?Š©[J×Ô8?³øҎÀ"'?¡\"l¾W/?a¤¾C?pÒ8Y&O?DÑS"‹dS?50^€D>Ë?‹NM-±ô?o~[,î?íýj~á?­èÓo|…O?…gÅÐþ7?"0·Z?ªÏs¹=×Z?¬4ªäg¯?Rž?›|ÁCB$1?n(ÒLù¤?:f:ÁüË?˜Çaèx0?˜¬ö‡u ?ë&©¿xó©?ª¤ðK^8?Ž-ôý9ôe?‹)Õåšç?Á'y³[rÔ?©o…^y2?îMîeMâŒ?'yXs™É?hÔ±åÐ?b9!‰eŽ?© Œc6l_?´'±W'FAGN4FGL J1642.4+2211¿ï˜Fé@BÝE¶ÃvÀ;rŸ'*_OÀ<£fô*ߨ@!"…]ÓE@°"—©Õ?ÏWŠ€wË?¬"OÓ|ê6?äØ°?ù?G@ž×ÈSkb¿îj.Ýc?ïü_#¦ù¿ëk><{±Q¿Ìm«ÿøž7¿á#ʪ³Q¿Ò^³ŸTC¤AGNbll1RXS J164220.4+221132?ïŵ¯'lµ?n6¢ëD?Fn…'@¿?7wV±u¾?zWeNYÆm?mUÖmU?﯈Š˜?€ƒ?XkvÕL2Á?b®ìÔ_[?õIüJ?y-¢Ø	$?ïR¹‰+À×?ƒ¯Ìþ¢:.?dÇÍ<Z?fŸÕïs¤?"î]áʚ?'aFMŸË?ï¶?~ÿ¹×´j?r7×~ã«?Y®òµ¬W1?™[Gâ2]Í?~td©Áe¬?ï–p&P>?|S©ñ¸ž?Yµ–¢à¿o?QÑKšYÉO?‡-C8ž?z¬ìº*l;?ï7üPz?"¡è'?Ÿ?e°}G?ov^£,?–}.֌|?' ŽFÓnÀ?îÌèŽÒÉÅ?æmÕ
?k¥±zƒ?m±œ"i?¡w&´ìþ"?Ù£€ëPZ?ìô x<ôõ?š‡{sŽ¤?Š¢U?|.`Œnû?µøÐim?šŸž2³ñAGN4FGL J1642.9+3948?éا2MHø@Dz'öè)JÀ89m;l½˜À;v†eà/@åëÛóÛ@dŸ¼ÉJ?£<!Þ?¥9w'.?ÿM€k_Ê@;ÿ>¹ú¿Ä©$&%Ä¿àXÔ!Õ½·¿æoP»v­¿åø˞#—	¿æ:%6ñ.¿àpë$¦¨vAGNFSRQ3FGL J1642.9+39503C 345?ïê2.·‰«?a"9©'y?1ÔÝí4?$áA2?c­¶¬+ñæ?`"D«%<5?ïÒUÁcÉ9?skÛ´³ß?F*‹8+#¸?NFž8»W?tÍóQgš?q°™yYüT?ïrTè~ræ?‰ü<ÉVm?h\—éÞ±?v^|n-?S¿zع?†>uå"?ïØɋµç?WŽÌægóm?SJM}QÅ?<š­	t?nBúˆï–?TV@MªÝ)?ïιiƛ?pëçÁY??™/Cz'Ð?6^¥G~.?v©¸™Ʋ?pAæ'Zm¥?ïr_I?¥zJ	h¨?\¶ÀÑÀ?f'–Ò¶7?Ñ{®N'?‹X2'6Ô?ï (^:jW?'sD¿""?r9ïcWÃ?{'¯üÁ3ø?—lxbã;?´Ó9²?ï'dÍù·U?w·@µ.û?m@¬oî{!?[ÀÏGŒ?Ä?"¡^·Sê?t¥Zë"–5AGN4FGL J1643.0+3223¿í皈×Õi@DC,¥zxÀ:»£?4É5À<#e_Ö)@ð¢S&˜›@üÄÞÁÂ?¿ôPßÁq$¿¡¾ò!M¶?áÓÆÞ@•Æ5ƒðe?ïôŸhËÆ¿éŠÃ=O¿â…yA	Š˜¿Ý|þ®F¿í™z"¿ï÷Ê! áøAGNbllNVSS J164301+322104?ïhšïÁ)½?ƒ<í=\æ?v]YÀò>B?j'3G?Šª—6˕«?©`xÉ?ïŠÆ£Ï
Ö?'=fÇî?eÐnxžÄF?iñ…ZÉ­d?‡Ú;zsqc?|]ªp¥†A?îú'"b3/?ŒMY?Hˆá¹¹?€³¢îÒ½?˜w?m!m?"–¨OIQH?ï*2Œ"?uQõüÖÊ?†U­ƒÝû?iGڔË{?ãŒ]Å"Ì?mº²•'gÎ?îu¡‡40?Ÿ@ËÂΫ¦?Žç*.c¡?ƒWÚW÷? ìÆä?œ_ñWE·?_Ï7O?œ"ÿ0@Gj?w#n9Ü#?€õYúãe?¡#:õ,?˜Ø•oø½??îüçfµ?˜	À"?‹bzã9ån?‡5(´\Ç	?§' *réX?"ÞT?í6‡=Bøð?"W2'*Ío?¢¦ž(¹K?Œ¹ÐÖñ?©ðî%z?FÂÖ*£ÕAGN4FGL J1643.0-7714?ï
‰er`À3æ‰enï¢À:Ϻ×5À<*•Þ#6f@ì¾ÝöÀ¼@$@Q(ç?ìÛÀ°Š¿¥IÞ}â?äxdFÑv?ÿIkjÏ?Ý퍁Þ<¿Õgˆ$|61¿ìÍÛ?¬=`¿Ü³Š;WÄã¿Ð¿'zç&ë¿ïÿüoQÇsAGNbllPKS 1636-77?ïQn%]ü?"µ§¼6µ?bï1}Ã?a‹kM"Õ?"tU7K
?"$Ѻ@ƒ?ï¥ÄÞtr¡?'°Ø¬?^.ZôQÒÚ?g'îbEZØ?'Èý·µE?~­ÔSô²¼?íÖÚow²?Ÿ•¸¡b3þ?uHÈ_ñ}i?tðma¿z?¯é?ûÙ¡?Ÿ^¬Ãõª?ïzù›añ?x€I¹¡ê©?bØ³Dlj?O¥öU"òÝ?›>å²»˜a?wX~JÎz`?î»kú,´ò?ž"KDE+
?yÀéN–›¢?vÕ¾ŽŸ®D?¡#3£Õä?›«÷cPÌ?ïa@æ?oEbS¿í?q[fô!ð¬?"*Œ2T?™%ºÌ!?šø':àÚ?ìòOÎõ?©bGæÒ5?…ù¢<B]?'`zÇüîP?¼Ù;E%y?¨He`·7Ö?í|6²Cµ?˜Íç"'$Y?€úéÆÒ¿¯?uuk~¶ŽÒ?µÔÁ´†¦?—9©kŠäAGN4FGL J1643.5-0646¿ÔTÈÔŔŸ@8xoš™tÀ:/<"댫À;ç–{(@ 1"­ú#È@
*áU?À­ŽÙw*.?*äâð?ÃÂ
V)ØA@ÊÑGZÝq¿»z£à…¸¿êßJþ«í¿å.iՆ¯²¿ßµ×<è=¿ä?z™¤¿ØÊ=fAGNbll3FGL J1643.6-0642NVSS J164328-064619?ïïÞØ%G?P9Ç(Z
6?3l™ˆo¾Ñ?$ùŠ1S?[g),è¢?N(ûÜá>?ïÚ±gt6?mÓó"¨Ag?@¿0U/֓?Jÿ©P恈?pf5Ñ4œ?i/¥ñ'd?ïLA+eÖÁ?‹Q™òý/Ž?^!ÂP;?bx²uèÔ?"•ÉwП?Š'œ{Œ?ïQp‰Ä©?obcltê?NËBe«'?0Ï~@+4?"çWÚµØ9?oN7.Êã?ïÞ¥'@ý?e-¬ö¢a?BMgùöý?5zv׃o?m[—-ì?cóg²ü®?ï•Ü¢F«$?;ûÞÒ?O
êV@"?[\C2fÒð?ˆ—øÒ¾'?Œ¨m|ÂÕ?^5ž?—˜Çð·Ê?jÉBuÂñ?nàvz>5I?¥š[#{Õð?–a:²¢b?íÖNE³=…?Ô‹¹ÛN2?h'¾"R?Rî>òç:?°‰Fo-¾?¾ö'œcôAGN4FGL J1643.7+3317¿‰¼BXB ß@DÔk&¿‡À;œÑ¹ôƒÀ<æݝÕh}@"Yp)]Ç[?ó1°|4.?ݜöZ婽?ïþY!Yl@ÒÞ^ň@%4ºÇ¼˜?ïý*BsÂð¿ï›iGÂ6q?à´®ÈÕÇG?ᇆqž©¿»f͔ré¿å×táSlAGNbcuRX J1643.5+3316?ïÙ‹ª?´šèsþFÆ?}ª{Ã?—
yůE?"ãhVZÊ?°"aPÖEí?î¶+ÖGŸÒ?¦	×ÊJÊ?{ûn:!?žÖí$?¬?˜¾Át¾"°?–W"õ®G?í½wl"?Ÿm±?oÛ?ðV*3ND?ŒzcäÏú‰?¬¬s¸tÖ5?›‡]لS'?ì¹DòDÍÝ? 0¢Ñyû\?ŠÝ)׸åÄ?Á	Ï$~"?¶Ú32c?ŸÝ«t?îbýS…ìœ?¦¢l̽û|?'®ñÿé-?œßGýq0? ø±Èˆœ&? Œ+Ÿz‹
?ì}:
ñSH?¾hÜãE_0?§kE§·¼?¶>Ã/úu?°`ŒÕ{A?­»ÿ,íà?슣€‰c}?¦"&‡ç+?‡ét?›`?ˆI6"a'n?¸­µuyF?¥]ž !o¨?æðˆûö?¼=¾/-ș?¢dvüO‹?£Ü©"Fy?ϤÂ'édC?»ø0"E'AGN4FGL J1644.2+4546¿ãÒ}은7@DkŠC»À;hEÏ)èÀ<ð1Cnê™@ ºÞ؁â?ýÒ¥Ú¼j?Ȃõ}Åþ|?–g—á*?Ñiè;")@aÒ­âQ?ïï=Û,áà¿ãÃނ׶¿×ñʳ!¿âo‰û–忽àÿ´«˜Ë¿è-Ë_\ªAGNbllB3 1642+458?ï«ÃwZ÷À?xgL‹»ì?I{-*¸t?<¶0­lF?ƒwoa…€±?wªqͧ›?ïˆüˆ§.?'Ám"a7?`Yêòo¦.?dӁç?‰ªc!¯ø?Ehiö¾¹?ï3 çTº?"ÚüÝ®ð?b/È0Q ?`9j3d¦?—Uÿ&kmš?"ƒSƒ¡ø?ïƒÇ›ñžÏ?n0aS sF?Vʒ…µ(o?AþÝÛt=?Œ4Ƹ	?ni¸.EêÆ?ïJÙÀÙ­?"ªÕÝ?Zn "ŠâÉ?O~•%þV²?"ýÝßñL?Œ.ùµ¦z?ïÁ]­Û?œç'âŠ2Ð?i"}cou?uµ*D#QÞ?œc"žZªŽ?š]¹Óý–å?îR´1½!?•Lƒ…=ê?hcb"Ó??^;°Þç?©N‹…B?"™Fí¸\?îWŸÆ{ÇC?eI8‹À?mº'©¤?aBFZ²?¨ªZiÕr?sZKÃ%nAGN4FGL J1644.5-4602c?ï…ïç•6¿Éýw¤ý%À8…‹W"<À9ï–
óފ@"#ÆX¿_@Ãûå¿?Êu´¸,?ڄ]<œ›@<Ÿ¡ñVð?øtÊÒ̖¿ïûŸH/Cº?ïåRj0'¿â8Y­ñ?s¿é˜´—Ká¿ïÿý±q&´?ïÿŒýÿʦAGNbcu2MASS J16444975-4559026!?¦—¶?°¡¸heæ?½½°O=«?Ã~<óó¤Ÿ?êò¬'ï:é?Åé>°mà?²¢Œùee?¶ºBâvÙÛ?ÒGVÑHª?Ä145;Ì	?äˆ\Ïþ?ÄO¬®§ÑH?³öÉÚmãø? ÊéKGKû?ÈRžÔÄ?±4'D<šæ?çz'͖ ?³Y·5[¸€?"ìj
°"?ÏòSì|›?Âj"løÀŠ?¦¤=Ï}Ýû?êÄˁH?	?¨ª‰ëv' ?'TÎóÊeà?®†/åóO?ÁÍÖ܉ò÷?ÅbO±Õ5ã?êùãÐì¹t?ÆÙý
y?–]øX\m?¡ô0PFW?؂žO?ÌSp¦—j&?ã5Ëòe?ËéÜnDE?¬'&̇'ˆ?™Ó7O@'¿?ÇÃ)=™œ&?²F£i+\?èFCÃh?³Tœ†hL`?vÈÓ÷-?gáÂë
?ÆÛéFkÄ?µF³Õ›W©?êtKº$?µ¢ò¢Ž#³OTHER4FGL J1644.8-2154c?îøí²J•z@.}¶™"¡À9ώ—"À;VqÐý³õ@ô¸ßÚñ~@§¸
è´?Ä~eá†BO?©©žŸgäÁ?èyØÔB@ÐUjÀ".?ïþ'ýž%ð¿ÛåB{¥"¿ä'Ö÷ÈùÙ¿æ Üš*¹¿ßr&s!á¿ë†hšMAGNbcu2FGL J1645.7-2148cPMN J1644-21560?í¹p³‹! ?§	â ×M?cjb$ZxØ?V ‹KÞ/ã?±™'P¶W¿?¦Õ—Gñ?î›Â ›bê?¤¶†5×?~m1ås?#‡¯7kÌ?¢v2QÚêÒ?£à•þð¼?é,ð:²zÞ?­»DÚ½ŠÁ?šVßçn?/ƒ‰"?È~¸Ë@¹?¬»U7|?ê™P&Å!ï?š?"í´å?‡Á×÷tW?gøøc!b#?Ä¡å²:¿?™},Åh¦ô?ëVi?¶1I§}'Ä?zIŒ³0?qçD¶?ÂÂ=<KŠÃ?µççK+·?í\y䮧?´nl`¤¦*?gËÔì<?–èF}Hó?³Ë)=ê7?²s³H²Åf?ã=Gû†Ž?³Ü↬ÞÄ?¨ ö«Ô•Õ?™Õïü Ò?ÖqQ2ïãË?³†TVqæ?ãƒ{X)b?­=XŸ*2?œ6—¿ð]…?ƒó›—škÊ?×5 {5*"?¬÷J'´óÉAGN4FGL J1644.9+2620¿ä©Mü.±'@C.}=BÀ:T¨ÎÀÃÀ<NŒÂÂ#@1:¥mbY@ѓpŠ¬—?»ÍÆFö´?´"»;)÷ ?ôØ/ž‹q@
öäñ0Ú=¿Ûdï"¸Ó¿æ}U–4Š¿ê"n§}‡ë¿èç2^wÿð?ïÿٟC&ÆAGNNLSY13FGL J1644.4+2632MG2 J164443+2618?ïøEM*ïÝ?D7÷v
'?6L¶"5¹?1ëE§}p?CÄqR•?=è-ÉtÚ?ïÈ?wTW?}øÉò©2š?TŔ–ôÒf?cªC挍?v®ßJِ%?vF©MéÝG?ï¡&V€ë?}'Ÿ«¨¤?eì~y¼?f8ٙD?'s»Nû.Ã?{Ô*¾2hÓ?ïêF縃?I<$ðq~?K>Lì»±?4TQ#…‰S?]ÔÑâaÎ?Cˆû%ä?ïó´É‡P?O0
&'Õ?CµÇ‡¹Ã?@û~'"ÆW?Mw
ûµ?F÷;ŽK?ïRØØ@?™Y÷µ\,w?d"MÝÕôï?xÃãú¥Ë?"+Ôo-ŠR?–†ù*$ê?ïT~—0N?†56:&D?p'ÞÎvTú?n†+)ƒÄâ?'Out{pò?ƒÜa(²¦Y?ï±lqöÅø?p~¤BŽs·?jVÒ¾4á?]Y‡Ç¾QÖ?z] ³?h4m'œ(ÏAGN4FGL J1645.6+6329?ïhýتÉ@Bü½º
RiÀ9á07Ö0#À<hœo6ï€@T—Äw#@
‰ÎÒa?´¯[ø¤A?ÆãÛÅ~@<œÆtÃ÷@T)`vP¿Ó‹¾úýÚ¿àö4êK¿æ,%!øxL¿ë´×Á¯b¿çj¯Áy1š¿ïà18‡0AGNfsrq3FGL J1645.9+6336TXS 1645+635?ïïå"¯‹?R ó¹ª?I6òý7ª?BJªÀ\ª™?Sš@¦jåµ?JF¯ühø?ïפŒfÖ#?vš·¤c!?HC"çÁ?T]|/—òv?q%G_ŠV?tc0݈©?ï9I>Q8F?œú`ԍ(?øËfß ?¯AÇV³n?ØÓÿ²g?‹¦
ï†ÛÞ?ïìC+	)[?B™«Á·xÌ?M³‰*M«?2ˆŒ³ý&?XŸåß}‰…?<žúü'è?ïææâURË?`J5&%?R¶ª¶ÌT?K|ô‰;?`B@´&–?Xu-Qw!?ï€ސ¢-?'ÐÞJÓ?Z¿­G}ðT?fÀÿÑ¿Jb?Œ ÒÀN0²?'-ܬõ´%?î®nõµ?–Hù[¾E?{?‰Æ¸—¨×?š&¦F¡;?'ïQ,ë?ïÇoÑQÊV?b×`ݏ	—?e	2À†í>?RæO6íO–?qÃ}üV¾ƒ?\Q
¾vt.AGN4FGL J1646.0-0942¿à÷´ûß	@6Lp¸Ï¿ÆÀ:¬~T–ZÀ<®Ò@!2ëÇ@¦¶~¡Ç?ÀÝYâÊe¿©—ÿ™jË?êᡥו~@":îéW¿´Îž31ZÁ¿ìÔ)þ+>¿Ïؓ)'ög¿çÀXëS '¿©à¡•ø‹¿åý
a½_GAGNbcu1RXS J164602.3-094113?íÙ*R±J2?¤ÞDÞö'â?v¶(ƒœ?iËwÝ90?¯–•ÓóNð?¤XøÖË;C?ï>y´?¥AÊ©¼?v㷽΄–?€SJswa?™æ
8ý[?¢÷³F
?íòH6GF?™p¥»ƒ&Ð?€;…uøæ?€®Þ]™o?¬Ì›@(•?—Ô[°œá?ì†B1RÞI?•´Íål$?eÃu%hÈ?UÞEÒ?»ÒÇýI?•¬[gãG?ëŠUÓén?´Ù2jáJ?ŠçÀ ʃz?ž#ÆsŒS?À(,­:¾Ë?´p~kã?íá¤Î^¥Û?²=ëðiå?'âùC×$ÿ?'ÓZ'
Ra?­,ôÌ7?±	{Ù¶¯?ë˜&k4è{?¦‡£à¾s?Žwù]då&?†Ôû¤¹xÖ?¿oÍz>,?¥Œ&ž¸,ü?åU(Ӏ<ž?±7˜¤zhê?~Òª!ö ¸?x"%¹.?ÔÚc° é'?±g€+'jAGN4FGL J1646.6+7422?ïçƒ'¿á@A$'žùTëÀ;^#QA;À<ñÄ>ˆÑË@ï·=ïNØ@=â@ÒX'?Îð颜Ž?Èùª¦\J¯?÷ôt{Òß6@˜5ÁWú?ï°û€>~Á?Ù=B äfœ¿åoïaLK2¿âhˆ•â¿ä²¥¤i×4¿áþ·á-VûAGNbcu7C 1647+7424?ïÐ
´¹Ûƒ?"Ћ»c¨?V"•õ«ÙY?dþ¯ŽÉ•	?rr5u{Ú?ݞÍÔ=h?ï×´Šš'?p&˜âæÇÑ?E¼ˆWöN?NæwnzŸÂ?qnd!Ī?j§£‹ø~§?ïL Tsʨ?‹ÞüíTkb?juvN	$?sÔA?"QÀ)4ß?‰£)ž-)?ï¾³ÿ÷Fž?ZuBØ-Ý@?fþófBÂÜ?I8À'"Î?u&†@
C°?V¸Vî+F?ï±1êoX?Þt¾èŽl?_J¿ø<?^7Ö0ÒÉz?¦ø0Œ'†?}€(i3ªç?ï',ö`?ˆ¶ôéäo2?\b³ñ5:?cYÓ]$ê?‹èx9½t?…ð"UóN,?îÕz˜ð?"[œ;"¶?u>-¿®9º?y	šU? ù@äšË?'3KÁPk?ïS{ӓ™?w©!a¥"?xŒ¶™q?d¶ÐÖH?ŽÚ¯ÌQuë?sÍyoS‡(AGN4FGL J1646.7-1330?ޕpo~½ö@3õZž²OÀ:ΐTvyÚÀ<)VlGQ@"m@JGø?þ¼I	^N?ƂcÇûÁ¿—ú¹š?Ð$ñüÝ
Ý@/¦(s<?ïüÇ0«™v¿éó5ò*T¿ëOŸ_¬8?'3CaK¿âFîœ*m'?¯¾
þV˜ÏAGNbcu3FGL J1646.9-1332TXS 1644-133?lÿ?¥¡íàt¬?~ADÝAqŠ?™y-^)˜?¡ÍŸô7Ü?¡|¯EUß*?ïiBWyŸº?•Pþ'p?e…_A+]ð?m·ËÒ´•?'	*â[ô?"(`A?W²?î9KVs2?šI‡ÂÞ_½?gyk­¡Y?lOë°Q¾Ò?ª÷ôŒ½Õ?™ÿéQ4G}?îË+2;o?†-;ýq?` umJÊ>?LʖӎDÜ?¢CE"Væ?…Ö},ÓÀ?í™þÄ@·*?°.)@è"Ø?jY€'˜=Ù?|ÀõpX?²]=ÚÂ]ý?¯ñ1Z:ë?îËl;"Ñø?©2YKNF°?lsaÓ¯ìú??{þl™¿?¡'3ƒŒ¨?§Ó\ªm)ä?ì¦.êñrk?£d—Ø"Ð?u,rÙJ6k?zÃ%¿ç:ÿ?¹{ÁyÁéÃ?¢ÏWûñPÛ?더)\®?¥zŸ'wq?~ú!x±{½?t!-;?Ñ?ÀÑÞNÕP)?¥sëUNAGN4FGL J1647.0+6040¿ê‰+"½È´@CAÚßµÝÀ;s €©ÌÀ<Äæ©å@àfgh@±ì¹ÒE?ËD௭­¿vÓÿŠÓòË?¬1¦|g?æ@5=†Å¿ïÜD¿L±‰?ïRuÚ¿èsûÿwD¿Û+κã–=¿äèÏÍ2MZ¿ç‡Jw—AGNbcuNVSS J164641+603930?ïژOË"?tuªJš™¦?C:-½¥Š?F§úöâ?pL—#BÞK?rº&Çà?ïàEW¢ÿ?kSËI¹?@Ì©ºv'I?I¼$•Tö/?k‡}¬ðú?fð(%r?ïo UKœ?~$å²âÃí?eGèQېo?k»ǪD&?Žåð¬NÒ?yº[é`?ïØYbÇË[?QU¼lѾ:?P£+´b?3¦àø-KŽ?oœ"ê›#c?PuþOÌÕ?ᆭ××Â?w™·þ` ?KnÁA€M¾?E«QLF?}>¼D9£ä?vt×MêÍ?呂Ç)Ž‰?''²Ûº?M"zŠu0œ?V='˜Ú"?"¦Žx?€¥%šÂ"7?îöf¼L¡ï?ŠmHTmð'?q¦.òî‰à?s\}ÉYœ?œÉœÁ—9˜?‡}'jtŠc?ïN˜Ù%?pߊ¬þ8?dٓ*Né?Raøƒ?†µôòon"?oÏ\tAGN4FGL J1647.1+6149¿åG EDØ¢@Cvÿ:Þ"À;AºrW5qÀ<éegÊ@:¹•?úƒŠéÓmÑ?Ôª;þ2öL?ÔzJ´Y8€?ûϨ´¿Í@G¢ŠY
?ïý#I±$¿íÙÁY|¿Ëì쥿ÖÍ.œ=¹¿ëuäޑpU¿Ò|¾aÏþ°AGNbllRX J1647.3+6153?îy8¿Jil?ªX³Y
º?I	Í ê–?žÛ¹îX?¤ƒRÑÑFï?¤ «Ô×¹?¨ý æ?åÕp»Ñ?cjBUm?d™	%> ?…Ä…:ý?}NLa«?î\K"Yí?•¾<OâLƒ?ƒ`Ò¶Z@?€¹Ú¨"ËŠ?¥cǃ}?"5[#»?ïOlúw^?l`lé@­'?p,ìLbè?RÞìÑ!_¿?'òêÅe?h¤ZÛï±?ìùŸ3›?±˜õYú@?†mOž)Êt?€ñgæ3H?µe\u'Ȓ?°Ð©Ó²öá?îì¬ï•WH?šµt/k—B?rQ³ê®?}…þ'Î??ÕõFfâO?—4Š?íE$rH?£J2Á,â_?‹f‡!®ø?†9½ïlèi?´1›)«d?¢]è×g??î)ד5'?Š9u"´
x?yÍÓÙk¡¦?h"+ʕÜ<?ª(ÌQý£¯?ˆ×)_.j AGN4FGL J1647.4-6438¿ÁÅ,‹_€TÀ(íêî ¬À9€éNã'âÀ<fåè&Å@4$ÕwkF@
¿@óW?±.q,"?§(¹vÙ¦?õA¼bò@ˆWƒŸ‡D?ïñ?Ù}¿à"P&‰Å¿å"ÈL4‹ù¿ãJ=Á+®Ú¿éˆŽ^Òô.¿§™(¬AGNbcu3FGL J1647.1-6438PMN J1647-6437?ïël=á?Vì€/U?<1^¨Û©5?.;+ZÙ'?a
Ìèï¡È?TXÐíÀýª?ïÚÁ´Áð?v°ôØ?@[™SF&?M€à´øŒ¬?p"²ÊüÕ?t(³^ÛèR?ﰚ]þ|·?qŽ[-Ù?]d8Åšz?b'*ÙpÀ?€,áeXDö?m{_/š?à[}ˆ?aºëßCÀG?hî­LÊÎ?GV¦g
;Ô?'`ܔæ?]Í8è‰Ø»?ïÓáµMeu?iH–I"~ñ?RŸN"‰?EVL{#?qgQÊ*a¥?fZ³_üv?ï 7¸¨þf?z@NSéð?UèÜMú?jB‰Ÿsö¹?…Q°)†"¸?~iOçÏ?ïVþ¥ž?}
>UõÛ²?g¹fjüxæ?f¢™^썝?Š;æÃÀu?zFw‡BÎ`?îäo¸—2?€ÿwóð:Û?'ÈR ׎Ž?gUͽéª0?š
ßÞï±v?|<náV<AGN4FGL J1647.5+2911?îdÓð
G4@C='Ýãu†À:É@š$À<gzbœ­@Ë["l@{k{y"?½†ý )Uº¿¥2!BùWx?è:±âe»F@öü¢R{¿ÔÖß?–¿é£(Ž"ƒ¿àSþO%Ø¿çOÞk…µ¿Ò34	òÈ	¿â^"3N&AGNbllB2 1645+29?ï̧‡‡¸
?rÜÑ8æR?P^Çë½Ê?A9k¦\ùp?u©d"•U?qœ»Ã«2?ïÛ@OrÑP?iÈøWñ'Ó?@
¬Q? ?H
ï<™,?p^'ÑZíä?fBd4?ïrðhn?{sùg?_­A)ý?U¹n*êâ$?"ÛÉTo?yï"0!Ӊ?ï×3:%Q?S;.¨×ž'?F†Òp¿Þ?1»'FUÉ?q§&#òú¼?R‡µÎ$?ïŒð'Ü[?…‹£ {ׄ?b#D8û/r?["Ðâ?ˆ;y??ƒ¼°Øùùz?ïå®E"I?"å,¼þL?P"`M}KW?X·–ÜZFc?‰ô(^Øx^?ƒRõmòK2?îƯ,äö ?Y30{q?nVàɛJb?l|xEf߄?¡¯Ÿ%°ÏÒ?F»_ÃÞ1?ïrj7£§²?uð!3ØÿÉ?aiBmÈ?S­D–dàD?!œ1úN?u=ט*SAGN4FGL J1647.5+4950?Ô^A{—ÈV@D	õ­–¦ À8ú'ûnjÀ<GùsôÄc@Ô)«|ñ@î¸D‹Ñ?¢²o~hß?Ÿ}ÀzNŒ?ôQ.ül͉@3L´äx»¿¸þö?·Ðç¿âíæÝð
¿¿æñਠñ¿äìö}Ë1í¿ã¼¡Ü^:H¿äÚ;JXêAGNbll3FGL J1647.4+4950SBS 1646+499?ïóïçë?OsþäOY?)S?4Ó[˜"x?TýfàFd?N‡p'Ö|\?ï×#"üô)?p_(²æB?B=ÜÃ~×Y?K\(–r7?r&yël2Î?l™MÆØÜ?ï»é¬Òw?tRlÞsh?T8«íË÷?XipóZ?|ý$hø	?s ãòM¥Ó?ïôŸÐ¦‡O?<cÞF"?CÉBSþ?-kQ¤æ¾?I½3`ý{?2(õµ"?ïä *[¸?m¡˜Tï?6b–Rx*?4ý¼Åk]?i2'd­³?jÚ
öj"?&"á›?ˆ
"Ì_sì?W2üâ€F™?c?qMSÕ?‹´Ê&<E?††pÒ8/?ï†Ó8A¸?';‹ì$7?]â»væÉ?_â`#؏?ŠŽÚ–Žn?Î¥A$?ïâû¡»@?[rg¬Y¶:?[Æi»'e?N¯d˜‡™€?`ëŽ-?Pq ¬5AAGN4FGL J1648.0+2221¿å8ñ¬2Öõ@BD±ëÕÀ:!Øb,EÀ<MˆGa¾a@¾úWI'ñ@7~0‡‡?ÁžsˆØ›?Ë$ƒB@† Ä0F@b=Í@:?˨c`øh\¿ãR@>´q¿é†k>'aí¿ç<ÛR¡"¿ïÿô¬å¦¸?ïÌ®.|NAGNbcuMG2 J164800+2224?ïÐ^XB?lÛ¥þbä?md1F`Äá?dB·Nz%?b=½¡õ×]?X­Ñ
"G?ï†ØX5?(R¾ð"?m¹¨Lαr?x"-AË23?†ÛÒz	&?†~º^úÑ?ï{e˜yø®?'ÜUô°Ãæ?zG¨ï?}ŽsåÒû?"…{*÷?sLò"5[?ï±fVêr?bèû²•?l­Ç½["?Q‡$š(g?y
 \qN?Zhä	EIC?ï¦	Âo"?~¹YX°ù?~Fço	S?x´w=˜·?mi*|Zx?iV|?ø?îÞûU¡G8?¡‡¡k­Ë?|ç€|Ó?Š âé7Ê?œæµ0lè?š)§Ç™W?îï4&‰gÙ?':SÐh?ŒR˜Ç=•?ˆpïp)¢€?"ðmeß?…j.§EDQ?îÙÎÅöCê?‡:—(ñ¨ß?‹ˆXÿv?v"®N®£?— ¢	?€muKI(AGN4FGL J1648.2+4232¿Ú`áÐÁ	@DË)^žÀ9¸xq*å‡À<wÜygË@öO+â1
@0‹¹F?±àÀõ~å?´
šGiv?ý œ˜Q›@ýuOÐ?ïÿÿ>¹ú¿àW¤ª²¿æg9ª€¿å9‡`1&¿è¾uñô¤'¿ïáãµFžJAGNbcu3FGL J1648.0+4230NVSS J164831+423322?ïҒdy¯Í?"ðºÉZI?EÁ,dҏO?PÖ!°
©?sþ¨QÄI?''tµnÂB?ïÞÿúC?l/1š¸?A^ž¬+Ll?JüÜÍî¿?l¨]ÑP?g¾÷†¦¢?ïuÆæëî?Š=ø,MÆ?b]¤:zVá?pÄ՞‹Ó?÷ÁEV¸?‡n5ڝñ?ïóNÏ´¢?;c=Ë3†?D"'Ž^š1?)uÑDškñ?N4*üÇ£?4ó*:yŽ[?ï°ôú	é/?"}¬	¸Ú?T€hév^?VbA¼†Ã?2´^G-C?'œ9¬Õþ¨?ï›ìû@}Ÿ?"nŒÌhæ)?SÎËw³¥ê?avßì?†Šç²Ó½²?'†êZöGz?ï:¿5#g'?þc´	¦U?oDÄP·ˆ"?vý2øP5Y?"¿€ÊDü?«‡æee?ï܌ôÖ½M?[[+Ä,ÖÕ?^x†‹M,?I>V(µé¢?d6Çô=,›?S³ÿÿYAGN4FGL J1649.4+5235?²ø,äôèž@Cĵ¢
ÜbÀ9*ÃÁ‹P+À<<ôE·š6@+Xäʑ@J¾A?¦?·>ßÓ?ª|·õ@EøÒåÂ@à?pXX¿Ü
²ûjo¿ßŸÀdµ¿âra ä½¿ÝN	îû̿䆃—¿¥¿åõ'ž}¯AGNbll3FGL J1649.4+523887GB 164812.2+524023?ïöŠØ­øï?u%*¹†?%L}dÛs?Æxçڍ´?PIdȃÁ~?u%
C•¡?ïÛùÅ:ž?kWñ	îBu?BŠ'rêg?JÇ:·?oØd@?g*ns''A?ïÈh®·…_?n
ÿÅÂ÷G?P÷kÅŠ³?N"ž)»ÑM?wÍ¸L
¨?lZll–ªr?ïï)|ŒSÇ?=´Á¥ÒH²?AèD îRX?#á
ÖOÄ?X¸åXök?8Ø/Å
Û?ïõî}í?EÏý`ÔjÝ?0GQˆE¬?#j"öµ?PêNùô^r?Bìæ{R9f?ï•ió}v?"·}Q±ÅØ?UhèÎx¥?`ýÐèÊ?‡øeú'Ea?'íïC.§Ø?隣eEݍ?s:êZ{õb?X·c-ʲ?WßÓåBØù?ƒOËiÕB?q@Ž™ÃŒ?ï×_ëäj?\œ ×ÊÛr?Uòþðúi>?BXݪ~7û?m§fsÂév?W<Ý9'0àAGN4FGL J1649.6+0411¿ïõêØj@<åý2Æ&À:!$^"ÖÀ<	"&¸Ñ@J°7•Ãv@ürâu«~?ü}õ#X?ÆžÙtzü?þf"¿?E@Ý\"è¿ïÿÿ)@k*?ïÿúÁҝǿé¥Ñ¶@™M¿âO¬{­¿ïÿþó…õ?ïó˧nnAGNbcu3FGL J1650.0+0356PKS 1646+042?înœÙü€?³
èc}¿#?Œ{s[ì?™]H«Kú?¢ӆ×~?±4PvN·?ïÕp€¬ÉÞ?rá<¡–8?Låïã­Áƒ?W%Í¡‹c÷?q«½»Ì?mÐ×ð€©Þ?ìÝûËèÌ2?¤KÙ_Æ?–ëŒ_Ý%Ú?"ÑT·`?³U>‡æmý?¡r±²E?ïÒ¨fï€ß?[<éXb?TÂD½ÝW?>!yõë)?q{;JYñˆ?W>w£î?ïÍèß/®?¡\'}ÎB?Èù€z8?–ч(?º'Áçü?—µºÊ\S??ï'dGÁúP?Šîm]/îÌ?Y:apwr?h´˜Z¢¶j?ˆ?¡ìÔs?‡X§ayW?ìjï,D?¥ ïV?œÅl¥'"Ù?•Qù÷ò"C?µw+à4†æ?£xvõ"ñ?ïzÆÌù¾?yÑO]P?oM#?^Ñhè̳?‰Œ9­Íb‡?v¢¼æ¢LKAGN4FGL J1650.3-5045¿ïÿÕfŠ‰ÂÀÈ þÀ7ã',"³À;ýº@¾
/=…G@žÞ|øy#?¡ƒfÁþB?§bܙË@ô6%UúÞ@aŽQ?ïûûß	s¿äT^¦ÿ^¿åŒ|Dôü—¿ä÷'ê)Õ¿ä˜æ€Òù7¿å÷>àæ_EAGNbll3FGL J1650.2-5044PMN J1650-5044?ï=¦D³õL?®¾îÆO?Vè«ó‰à?pXø+Ú«0?–ܬ«Ô‹†?¬%r,ý•ì?îžPk0Z?±Œ.sœ4?@»‰¬7?O²"è
v/?¥Ø(Ùç2?±|N¼óÞ+?íDŠÄ1?£oämÂ&?×'9ÒJ?'YtÀ?±¥èÓmÄ·? ýØU¾ŽÌ?ï¡óâ)D6?lRÙ5wÆ_?QEp=zíÜ?8gŒ<»?…ZYz¶"¾?k0öÕ?í†Î÷R?¼d‡½?oˆ;z`ã?à$1Qu'?²Ñ"w|þ?»''B¤Q?ëíôfç?¾~ƒú²‡?W"&k'?l{C[,V?ÀÂ07y?¾Y¨¹ƒU?ì+ü-ô–&?¥°²Xåò?'eHÑwxÕ?ã¼=ã"W?ºÌYׯ ?¤…/8•Â?îùèMÔ¹?¾ñ'¶?lqº†Ã?[_ûÚTÀ?Bȹø?‹iZ~ÕÓAGN4FGL J1650.7+0831?·ùtRe½@>¥¸fä:¨À9²rùòŸÅÀ<<(¥:¸@Ñ
NG6@Øró<£?¼¸«­˜T?Ãy§¶½ÁÂ@°~ZxòZ@SaÅ¿ÀŽ|2iµ¿æï<™
' ¿äE`ýpه¿ê®HÌ]ç¿ì1  œWº¿ïÿÇ*Ì\eAGNfsrq3FGL J1650.8+0830MG1 J165034+0824?ïÏÃAˆ¶r?pb$?d Ê
GkÅ?ah`ô"õ9?lôkaùË?g=byÛX?ïÆx³¬%Ÿ?xªÈ¬[Ý?Yy8ê?d1X/öw?veWùUË?pì§7ƒÑ9?ï›Ì°ƒ|2?~C¡Á5?oI^Ë¥™?u¼Ä1>Ü ?:|aÕ$?s™íÀxÉ?<=¸?eËò"ñîW?tíÖqa?S'õ7ûÞ?…3
É{—M?`í¿b¸PN?º"¢?ˆR¬»PX?}"S¬øã€?wbW@Dp?€Êç~ƒ°{?ƒNÏRu²?ïZýKg?îÀFêe³?g݌ô«Ê/?rIßôÿO?'¤¬ã€â?ˆæ`.¯d?ï:çšáö³?‹Eú:Á?|»Œ­R×?~}Þ[Ï6o?'œÝÆÅ Ü?"
~L@¥?îžøC6?†˜ˆVäí?ŒPތ4M²?t¸ïuCN?øˆ^Ö¢?'@©BúìAGN4FGL J1650.9+0429¿ë€š«â@<À%á;ÛÀ;Zœ-ȐÀ<r¹¸óÑô@!a‰óß5Z?ü«+­,ôU?ЮúS?µJ;"ý¾?æ5™e—4@Ð}
œË¨?ïÝÅB"пîJn×N0¿Ö4œŸˆpý¿âBá[Ð
o¿"*å(Z´y¿ç"Ғßk5AGNbcu1RXS J165053.5+043009?ïMàäù?""°^'	?Mîù)v?CU¦ËŠ"t?•nóV8Ò?"7/ù	D6?ï>CÁ+N?™0áI["¥?rå™ØœÏZ?vñDkãՇ?"~!hçg[?•ÖâËæ™?î×`T‡u?'Ã.%rÏW?a,heZ|í?Yt¥ÕÆ:?¡w4-ÈÔß?'›óÆH¿±?î*ú8&\?Šbç7å¨?\ÆË8T?HÅ£—F‹ú?¬j+›MôŒ?Š~	`@?îb£+qPƒ?£{Ö¢$ä?_SÉëðÎ:?R¯Wª¹?¨Û.õ—äf?£@oÈðS?îa¡9*T?«.¹aA*Æ?~Dbœ‹ž%?¡€Ê"?¦bõð;û?¦ï,›?íq>NÍÌ? Ãeb2äª?j69·R?d؀OƓ?³¤\Õ¾Äê? x¦y¹ÅØ?éùïê"?§ÃÉ>´
?qÔ>°½Á"?i>ÖcQD?ljžb3ÚV?§Õ°¦iAGN4FGL J1651.6+7219¿êl¾vÀ3@AZ*o?RüÀ:u¤åýö;À<¨ÃФÉ@ €ç®z|H?ýùiÈñuú?µÕáswñÔ?sñ‡l?Á«Ü<Vr}@bô6H;ƒ?ïӟ县Õ@Q~Í»_¿â#îâvWJ¿á{ý§`+º¿Ø"ÿ^ow¿¼âÊ [PoAGNbll3FGL J1651.6+7219RX J1651.6+7218?ïÌßÓJü?´™I4¶V?O'*Ž:þ?A¿—»O'¤?"¥qœ­ÿ?´`Å?ïÒ9œ—?q§˜Äê?CNŸýbœ?J£‰"œcü?t1ž #?oª`rMÓ²?ïJ@ò«?‰Ç¡ÈM?^Ói?ewÅü.?"Ñ]ú¼\?‰(
0±,?£P/?f¶¢-ÜÆ?bƒ_ÕÚeÝ?C
¸WpªÕ?"^þÅ?f€²T ö?ïr†þ‰ ?‹MdTë?`¤‹‡×~?U_Òo™V?5"ðª{?‰ÔqŸ	?ï‡8í̧?†Ž|Õ*Ï?T5"Ï U7?]yŸy
¥3?‹« >^Át?"ýÀ	Åц?î±®)YÑ¿?'ùיoØI?j›¨M¸u?løÆ_>b?£;bäs)?'ÑLkñô?îÅâîªÌ?…?wMÇè?{'þúæHp?e»XRöÌ? <Qím>?"ù³äKÛAGN4FGL J1652.7+4024¿X|Ïq]^'@Cb¯È°À:™":ÚÇaÀ<q.~˜ŒS@ Úàl'Ο?ýC$\֚¬?ÆuÌ4÷X'?´o"3,'?ñÙ«Ø`@ªÅ
¶'N?ê&둳ò
¿ãþÀZN¿Ï¥_ö_Ã4¿àXŠp0ꄿÜ®½î¸¿Þ˜âºtÛAGNbllRX J1652.7+4023?ïոЅWÝ?`y8‡ù?<À/Ȑ¨Å?(à]£»â?sW"ª/2¯?_P¯¿þŒ¨?ïÃ2[ê-þ?s4HÃ֖?LÜk uKO?NmxEsÿŸ?zËD©S©&?qœvß؇´?ï›ä¢tµ?s}î°[ÙÄ?TÞžLt?TTùSØã
?†kS˜SU?r®×‰K"?ï'y¡à?rlÜ>fè?g"Ž3}9 ?EM瞁¾Î?˜*Ÿ
ÓµÎ?rkøk Þ?יִüÏ?t:Mæ^4'?I½€cÀ?:)ғㅢ?ƒ`€ÆÖgý?s–§'FìP?ïpåö"qg?ˆïó¼||æ?[?s0¸?aÑ£ažŸv?/I0Úð$?†ÿDªe*?ï3,[íUr?"'ۊí¿?^½ðyñÑÉ?PÛÕ÷>u'?—®•}uä˜?ƒÇ¯‰ÌnA?ípHÉ-Â?'
oHEÀ?{1ìJE?d6½ÏTw?²ÊšóÌ»?'rÛP‰´AGN4FGL J1653.8+3945?ç)Nû22@CmZ¯xþïÀ6Ę¹ŸÉ_À:½¿_ü¿Ú@7o¡Îqh?û‰¨U?†?‰i<¯ˆÄ4?"hKeP‰'@
gý?[`@0''àCÍ?Ú+Ú佄Z¿ÕÇ+£ù[¿Ü2Ÿæ¿g¿ÖPñ_(Y¿Þ"ÊÕ{Ç÷¿ÏU)¶³AGNBLL3FGL J1653.9+3945Mkn 501?ïãp.	?e
âIt~?3÷«Û]äŠ?.¯\‡Û?jcšŒX?dc	‡Ÿ?ïÄ`')!{?z³Z÷yžÿ?L$W=Rr{?S¹óí%Dw?zK,d'Ö?x×"]*?ìôÖu[æu?¨EAq"Ñ?w¥40¡ñ÷?'nz£©x?¶Þù|¾½?§Pé»:Á,?ï଼û¸7?Z£Éeh?)›§[rù?.$)¤Äé?m¹ˆ[0É?Z!tƒcÐ?ï·ÊhˆCu?wŠÉ™§áz?CŠ3`,Î?8nx'öß?€Ô·b"Ü?w¶±íúJ?ïNρ–ï?LÀµØ¹?\[·Þׁ?g
}¶ÔÝÑ?"`TX»»ª?›û–<Œ?íEûż?ê?§õíÏÉ"ì?t%˜*X?‹'¹4n?´ŽpqWF?§f[ȋq?ïÑԒ­°í?l¡B¥U^?1n:V®m?)òáëÚ\º?uþÓ%E¥¢?lWÔ«PÖAGN4FGL J1654.0-3509¿ïêÛÉ@˜W€ðUhÀ9ª6CˆìÀ;'ã}zV@)Bnº@¾aÏþ°?½n'¥áP'?ªŸÀÊØM?ïºÿ?8$@Øד¥8ß?ïÿ®©Ì¿äÿà iA¿ãpWìPÓ¿à¬ÿ'¿çõò•´1Ë¿Ô©ãßVAGNbcuNVSS J165404-351301?ä~DŽŸ¦?ÉRd4÷J?o"Èë|œ?fê@›f¦e?ÖÄ+eUç‹?É8©2ø?ç¦õ¨?»^SPÃÕ?Žërj°Â?‰Ñ|¦ú?ÐÙmVgK?º ¸µœ7?éÁ®îëZ¬?®2ÅMÁ?U]QM?ƒZîýeÿ3?Æøy™¤?­¾fZA?êoÉڇ©
?"í¶§F€m?'
Æ[Tû?lõ®Å>?ÃÿÉÜ#ú?"ꤿ‹b?Ýò¹IÑôï?ij9à˜Óî?ƒA»K?ya¬±©?๞ø†Â…?ļ÷º½?ÝÀçËD¦<?Đ҄¶we?˜õu¯jÍ?œy@N?àW㎰1Œ?Ãåd(«b?áÜØwi³?¹Eßޏ|f? -ºí4þ?&rÀØF?ÛôŽò–:?¸¹à–@9O?â¼.ÑÆþú?¥ú•Î_©?¦Ž,þ
¾g?…ÍìÝcrì?׵ܼ•-_?¥#Ê=.iMIXED4FGL J1656.0+2047¿îü œz@A$äâmHÀ:!ãû½{ À<RNöÞ@-â´?¸'@ŋûKeY?Á'ï@À£?ɹÀ€Ž/Ù@ꇅšß@8q¼Æ¿äDFŽ¾¿á[©t0¿æ<ït—'¿çlãË¿ìK`†R"ø¿ïø¸®1×AGNbcu3FGL J1656.0+2044MG2 J165546+2043?ïžáJÄZŸ?xž?q­öÛ¯ŒÍ?fŽžr'g?~ác´d³ú?p<	p? Þ?ïÏRõ+¡Ö?sçnÆR¦h?Pl¬«MÛ?X#W0!?t;"]ð½—?n~
PèQ@?ïˆUµ¥O?}Wù¸QŽh?rÏȆ•P¢?qÚ¿Í¢?"'®GZðW?tkGja?å—I?b´7g8á?k.¾Hîb÷?JÝmˆ)·?€ò.4Ÿ?_I²ë–?ïô|¶S?œÂyÿÎÁ?†xš¾®?~/²0z'c?'E#XqF™?…~ÿÈR¬?ïr"9©"?ŒHF2è?b9K
Í[æ?k.·Àü€?ŽÐ¬3è–?ˆIx¼K™?îú~Ž{Xf?]*¯?…ͱ>Êí¯?Ø;"
nš?•ÉU–Væc?ˆ¼?îãåYNa?ƒ":)'è?ƒÑíÁ"?k"ÿ:&§=?™šf:u‹?NëîΛÙAGN4FGL J1656.3-3301?Õ@ù	k¹Œ@hH'ÓÀ8ç
ÜÒÔNÀ;)yÙ	ò@ÆGåœÒ^@Ršäó4@?º­j˜?Ót¯'@T+
oÆ@"4A{†¿Ïñ@õh¢¿ä^2.o¿ê¹Ë"}®W¿éY<a°@¿í-F¿×ñÄ¿ïÿηˆ—êAGNfsrq3FGL J1656.2-33032MASS J16561677-3302127?îzˆPŠËº?¤–•:0ÊÆ?¤á+Nnj?£I5Û²'o?€âg E#Ü?x;ûlgR?í´LÑûñå?³´§9…ÖÆ?"uK¾êÀä?Ž4¢ˆ¦cI?¯ßôMÃx?±³ÜÆ'Î?èÒØvñp?®.hMeFR?¸0Â\qË?£å‡£ŠÏ ?Á¤SoFgv?¨ÀéÖ"?íŽ&e&(?'}æç~t'?"´3¿A?xß'I®?¬Ã•€*=Þ?ŽÄËmôq¤?î=Dçï³?¨:^_V³³?¦sAϯàk?¦h	š•1?†á¾Åyѐ?"AžÎ¥	?ê€]+bÊ?Æ —;è°Ð?¢=]Ɣ*m?²zôæ6ú??Áo3áÑ89?Â¥ðE‰a?ç?eoÏð?²ºD› ¾x?º¨8‹ë8Ñ?¥w…'?Å®Mþ#Ø?¯IM"%ƒ?ç$z>›­V?°N³Îê'?¸aËXû¼?¡ã%ð"¾ü?Ç=1Yl™?«hatVlˆAGN4FGL J1656.9-2010?ÞRoêÎb@,5inX£À9j›‰]â3À;âxˆ§ÙÎ@ z—éJ?ýT¼ÕÞÄF?´³£(2ú?¸öª蟑@í^µ˜@J4Sï–P?‡µöØ %á?ïîÛJ>´¿á2"¢¶‡¿ÝœŠ$[©õ¿ÚºØƒA&¿àäõ¦n"AGNbll3FGL J1656.8-2010NVSS J165655-201056?ïܱçn8Ã?d#œ¹˜?>â"X$ $?1´ÌÅHÚ?oqÔ<Ýrä?bîŽrÜÜÞ?ï§BÉ "Ø?†.ÚÅ5l?aþö®[<N?mg<gHëU?¯ôÛé?€½-Ā?ïLìËMy?|zàº-??`³ O½?Pô¢2&9A?‹Ü»§õ?{H#6é.®?îÇ »aj?~A'µÏ±?ŽgB1èUJ?kÊΔ3d?§©½d`8
?{¬[!¬X?ï´wp`!?u©#QÍ'ë?UË
?KÎëµ"©?€U5aº?søm¤È¼?ï˜q·Žˆ?šó[ǛN?s`åÙÈ7¯?¦­@!þŒ?˜´¸R0
?—#¤:€†?ïxªX%?¯b͍c—?nêd?­;?m
%qnÏ?› $bµ×¾?ŽãŠU8SŸ?ëžÅ¼H_?–ËTâv¡? ÷¤n;?†.ãt,m^?ºÿæd?"°Õia?!AGN4FGL J1657.0+6010¿¤7êeڒm@B´iaÃiwÀ:~oPóÇÀ<¥ôõ
¸@™'Ǿ,@cg]Ý*é?¼¥nS"Œ?¢ôšàÛ;i?äXy¾²Ø°@
	ú
å¿á†*Qb¿âO¾Ÿ !¿æïŽÎd|¿â°ô>«·S¿é¬¶ApØ¿ïð‰À]¨¨AGNfsrq3FGL J1656.9+6008RGB J1656+602?ïõÀêt>?D¾7+~b
?;adV‰wL?,C}ñÔ_?KK¤ÂÝwò?@ï'qͪã?ïÞ÷áðÂÃ?o}Í.Ë0?DE|ãUõ€?O ³G?kö¾×¤hÁ?hÖç°æUÍ?₩c"¥?q"úÿ2K<?Wu!~Т?`£±êV-?zIqû>?n'ü™£ž?ïÝЗÔêË?Lڛ}å]?X/[Êm'S?8aõçd';?fºHž#÷?GdåµÒÔÏ?ïåj˜Ø²?ZYÌ£Qì@?Slºñ‰–Ö?CVejº×?`ß	k0Ì?Up)$½×Ã?ïŸÖ3LJ?ƒç
+£*?T	‹øy×e?a»3`	?…‰A¯8A"?NŒ«þÞ?ïŠöá?y›õ1ws¸?b ":Ú#|?_ÕbJ^Þ?ˆšVò™ÔÂ?wW,Ÿ3Ï?ï›w")Ã?m8=rÍ#?rðósà?YqÀÆ	é?¦Ž!{Ý¿?f"Šd$êAGN4FGL J1657.7-6120¿¼š—¬•°èÀ&¶"áÉ´À:ˆ™'6À;èZ§ìB´@>tà&ƾ@Nõ>M?ƛoG5ž?rŽÛ"T¥
?¢bÕã ÷@`Ü&$?Þ©'`ìÿȿꯍâ+XÉ¿çù¥=;ʱ¿Ù^–C"êf¿ë2ˆä?°¿€m»qAAGNbcuPMN J1657-6121?ëz²'êæ?¿˜ºBþÏ¡?/*´/P?w
ƒç€­:?ÁD–Ñ?¿ÌOydñ?ìÝlhø«½?³âœ…XÛ>?l[l¶"?qö'<ؐâ?¸1Ä$ô;?³o6uA&?ìäJÖ±æ?¢x—úÓ?†G®¾Š\?€$#€¼?¶³x4f†?¡l¡"ãø
?'ÿM~?W鴃¼£?hª»ÄSŽî?J{8ɵ|?¦IÁǹ|3?~6Q¡a|Û?蛴>5šÂ?ñ³3ý??‹Ú™éö~L?½VЂÍ?ËӅgwLW?ÃlJoԓ?麜ÃÆ?ā1Á¡©?tr¥¿bÆ?ƒ¤ŒñþP!?Èv÷ùKZò?ÄCÊŋì?è9˜ã[?±]¨Ò.§?™—©æµ?ŽóÖRÚ?Ëæ§5ÛÑo?°ŒN"xøƒ?ë\þ]5¿?›"%
à?ƒª£º×BL?m#¦|ÆÅ
?ÁQ\OGw?š×l]Ø? AGN4FGL J1657.7+4808?àI¨Sîh@C=½øôsÀ8'BhZ\mÀ;ü¯0ړ_@mE÷0"³@xÅÿS1Ö?¡"ßíª­?¼"N^‡Êº@	0¾
í)@q܂!ƒ?ßê
 AÿT¿âɱgì¿åù»þHoÛ¿ç	õíW†Ð¿è"9-H8¿ë3Ÿ¿£n…AGNfsrq3FGL J1657.7+48074C +48.41?ïëRl)?a
±ñ`Ÿ7?E
Áƒî"Ì?9™]4Dz=?^^z^À՞?`=E¥
™í?賈R¸è?EÞÜnÖL?[ìþpàÊ$?dl饲?ƒa‹{jÏÃ?âÚûð™?ï ®[Ñ?…ÆÕ£^¼?gkíÏ|ۘ?vú¬­kE?' ˜çnÿ?'ð¾qù?ïâæ¶q°`?P£Í×?[éíÿÐm?D/½E*?^IDœîâ?B`ï}הM?ïÙE~íÏY?lŽ	]kÔÜ?FŠ^oòƒ?<ềY¡?pšïNfÉB?jÛ߈?ïB#2?ž8w!³{?n{½Cúw?|技O…I?›HCð؋@?œJÁ\e¸?ï…T¯I.?Œ/éI&±è?j€RwÓj†?yDWxWïœ?ˆ
åk'Ü?‡¥ÙP»D¿?ï±#5åA?n¾9ñKÍ?r—¥¤šùž?`ü!êܐc?tÖ¿"Wő?d#>Ô3™AGN4FGL J1658.4+6150¿ìó]ýƒ›@Buø"»ì«À;
ºª‹YeÀ<ÖFô@>#âÞ1#@ _¼(9Û?Çõ°[R;?¬`j_*™?á6É™"{@([DŸAN?ïaÜ>ñ§¿ç_d¥Ï2¿áȼœÓཿÔ|y"UÀQ¿ëþáòο¿ïì=ÆþAGNbll3FGL J1658.3+6149NVSS J165808+615001?ï…VÎeJª?{'¿ï'>?gôݙ?Uµ!?ÙÊb?ˆâ6&H7?xKԀ$œz?懶núó?{ß_ʋ?^‰=¦µ©?ac‡_ˆ»?ƒ|Œ¢Î?vÕß}ÐüŒ?ï,V"Y°?‰#ÄêÐúÌ?r‡ù²«³?rY†³%ÅV?•îš–³z?†÷ù,nvj?ïS&(ïɍ?p'QS,Á`?}¥–ãhèõ?^#3±<^d?Œcªc/> ?j€ÅëSn?îÂ:H‰?—³žœp‹?xŽ¶Z¨??k±oì§~¤? Ø­+¥b?•þW<›¤?ï ê3‡c?"-^£r?jóàv¢/?qVÏm,¨{?˜ž&²v~D?'o²«¾~8?îEô[匕?˜l€6>^?~‹ÂgI?{ ÜcٜQ?§ÞÆcN?–PÖ¢²ž®?î®ÌÒ}?‹5küæ5£?"oM¬{â?{Z9ä}š—?¥-D•\þF?‡121hsUAGN4FGL J1659.0+2627¿îct-K¡@AªÅO±À:±räùê<À<Q
¯ëëv@7;Îßw@'¤/?ÎÖç,õW?Ò(ŠBŽšã?úð"!'÷¿@ßëR?è0ál—¿èt9rèU¿èB¤À>I¿ìCŒFÊ¿¬¿æÑü·v#s?¹`4žWµAGNfsrq3FGL J1659.4+26314C +26.51?ï·We?u¤p>)Ñù?]\³2:›x?Rz¥¸ãÃ(?}(Ð"'"?sl
gÔz?ïŠè'?žȳp°?†KÆvG÷?'7(¤þ–b?"¨¿Çî¦?L¼"-òð?îøE_õLâ?œœ-r©ì?+Ø´Á?"†ýSj?™/‰XLj?Š¾ø)Æ?ï# œ`Q?tmÔ¨9Ç?zãàÑò¿?\ÿ¶–@ÿé?"âôEP…î?pԅ'vp½?ïHÁ3€Nß?ƒµ¶î"§?kÑÆú'j?e/Ý€à?"m ¯qùì?ŠÝ©KºÔØ?í€ï}•›Í?²tXÕIÂ?–äÊ؇¿?¢˜°§½Ê?¬ÃÍ´N?¦Këî~Œô?í×J–Q?™" 9:Ç?ŽÈ^ŠGT?‡€Å?ªÙ?ˆíT ?•xAW'¯?줬ú
fŠ?˜<ž´#ª?˜<=EO?ƒ§Ã‰D>?´Ë–ŸßÆß?"¾¬gkbéAGN4FGL J1659.7-3131?ís/¨¢@Òø_øŽÀ9@Bæ.žÀ;'ëƒq9(@5ïù>@ðú#G,å?³ÊL¿Ì3J?µö<Ý«í.@=Õ%`â™@¤÷;
m?ë\ûÿr©¿ãt›Gï'ڿ收:º2¿Þo•¤—y"¿åeüH»Zµ¿ëÓŒÚnvAGNbcu3FGL J1659.7-3132NVSS J165949-313047?ï"*¦`–2?‡ªˆ²ÊÒ?C9èÜIÉ9?B±ÿóô?Š·ÊŽ?†Îš8"p?íèûaYë?®Ó	>!‹±?eR©º??p\¥" `?°
'-_KÏ?­¬úÿ¢þk?ïsEòÓr?‰öv{ñÔ?i,–>£ÝH?e'8FJk¤?™l€°N?ˆ^Ru?îL^ï¾X/?~˜Œ"¨
?†ZÏù4ÜA?b61xə?¥£]ñ_?{íªúÀR?ï
EC«ü?'-kªa?PÒ.Ø\W?D­î[Ò)Ì?±ï^™©º?'¶"x³Ë?ê؏Ž±fÈ?¾jيç?yÙBö¥†]?"
#opÑ#?ÃÎ÷®fŸ
?½£§©@ši?î4®% V*?›*"ñ?yÁíg£[?x!{}é×?©'%jŸes?™׶©­Š?ë"<Fœ
|?–ÁTd)vü? M±ø—ô?ç­g=C?»7ED5l§?"j´ÖkDAGN4FGL J1700.0+6830?âC!3Æï@Aš¸¾øγÀ89FÍCëÀ;ׅJW<'@Â]ûu­@:>xá"?›Zm^Ó!?ºŽTììQø@ÙùŸ"®ž@TÖ}АQ¿Ú Ä܏û¿á1ìv¶?ÿåÚò)}¨¿æóe½Éû¿êÎ[–x¿é\°9ïAGNfsrq3FGL J1700.1+6829TXS 1700+685?ï»þˆS¡?•ôà¥b'?c_{·Å¢a?]šËœmØÏ?xPýèz*?•á›VBÀ?ï£eêYim?ƒYpÚÐ?`'£"òÑP?hºSN4Ú?ƒ܃a‡?€¬ø¯öE¡?ïp(å…?Ž÷Žéӝë?z²2Ÿëê^?":ôìã?†œ­@²9?ˆ9Ƃ›?ïïÍ×a?EìSöìÔc?KT‹ªæ?8=úö}ÿ?Rºæ#q/?;uN¯«?ïqÒ!¿Ð?ŒÁúí¹°?p©Ä:©3?hBžZ¨}ò?‹""¨»9k?‰É¨¤?îù榟g? ÿV@a@£?s"ó‡°ø?'å
"W2:?›Þ?Àÿü?ž9•¤¡ÈX?ï&ÄUì?•ˆÙÓ§y°?}0PЉ1?'X÷.Ÿw?"ÛañQØ?'±2d°?ïÕ)áŒÇ?cÇÄÑ÷?aåŒ/ÒlP?S÷øæíö?hð'ë½?Zr¡6Ô[AGN4FGL J1701.0+6613¿ë,©ÿ˜Q@AÙR*o?SÀ9ì¸c­OÀ<y7ýO1@ë‡('çP@ÑBªŸ{?µ£*€ËÜ&?¨o¡"2
?í'Q;[÷@J¨¡tYn?·ä£Ù
¢Ö¿æêµ`I–Í¿è"œFó˜¿êƒCÿEÆ¿êí«i¥¶¿ïþ;âÐAGNbcu7C 1700+6616?ïòèº`…ô?NIÇ8è«??9ñ	fáÙu?,>0ÌóÉä?S²I•9%?J@µû‡H?ïÇú>cØ?x·Ç[6›?T"_3•Ñ]?^kCÂbì?wrë.µ"¬?re#h`vÃ?ï©'¼1Ÿ	?}¥5ÓÒG±?_r[_Ÿ¿M?fŸã¬­ˆ'?Çń䕾?{áý¨HE?ïÊôÓQ Y?Zߥ¼š
?k€´Ðì"?Q ς?iŠwâšé?Os±œQ?ïãÃGמÒ?d Ì³^Q?Hÿ˜Añj??`ô+j›?eüòP2Q?bv±–H(?ï`öC#ýF?R©›vt?eìð²ê?sÕ
PDl?'#™ ,å?Š&Õ¿«U?ïq´Iž?<-À´¼?fߒX¦ð?a)‡HV?Ž
uÈÿĹ?êG°z?ïP'¿?}:0P?ˆ—ùsƒaG?t#´¢¢ïf?ƒb|±bí?o`žØË?AGN4FGL J1701.3+3956?؀vœXTš@B¹Æ\pC_À:1!
;ÃÀ<Žgú»¡@ø˜¾ñî@2<ã¶^?ÆMO~˜a`?ʇò<ÈÞ+@£¼ÅîŒ:@GhÓ©	ú¿êZ…¢kÐ3¿Á‰¥…¶
¿áúâ‰Ít¿å–¸w«¿è×ãD8>¿ïú":½k0AGNbllB3 1659+399?ïy+ÿ"?'Iy›úSb?xtþñÿ4?x°ø(mÎå?…zø6
'¦?t®Ô¤žî?ïÃK¤÷¤D?xã>T¬± ?W_òÂ?`eï+Eé?x"ÕePÕn?r'ævW?ïab
¯ª?ƒ­¢W³¼?x¾S‡¿ö?{ځí,0?‹HS˜è˄?|4©M±?ï]‹û‰?j«'2!±E?FM>9³?Xv?±ªB?ˆùÚzt
J?e…‰*"é?îƒÐÇ®)ô?—ɾ¿1Èi?ÃmDÕ[·?‹ß^[X#?žÂy¾†-Ä?"å["£"?ïE^_öyˆ?'*$=bfF?n¢2q ¼?u=®a©Ê‰?"í¹_?‹tèzÌP°?î¶ËÅåt?'ݹhÌz?Œ9~F™üÈ?‡œ1_¯¤.?›	Üå®!?‰ï¯(?îd‡Ž ¶ü?†M©ûŒ_?'­>¯?u?™½T? á
 mì?'ßšH¯àóAGN4FGL J1701.7-5621?ï|
þ¬À!Œû¼¾bÀ:f/Ш# À;—Œ™¦@4›Jž´·@ >ê šª?È Br–K? "…`Q¤b?ܬ®^͕Ë@Zª=€¿?è›×âTžh?ïÙ_æÌR¿éùJn¹?¿è¸æ0K!g¿Î°Ý˜wÄ¿çë$ p¸ÐAGNbcuMRC 1657-562?à¨,àÄâ"?ÇhRb'5?wí'äj˜?pP=½Tì?ÞOïùÄôß?Çdôö:?èÌGîE^?Á'\žD,?|?ÜÈå¯?‰²(‹ÙJ[?Ëìç®iN<?Á"4ÅÁ?ä7Au@Hð?²²$èE7è?—¥	µ"ð?ŠfAW­×?Ö,zdþ?²uÌ}$-?ìVšv8k?–ÆÙØHâå?€ã
-Ïw?oCüüaÝ7?».Ê©îÈ?•¶­‹øD?Ҝaþ€V°?ÄVU{v\Â?‡Q¨ƒGV?€PŒOþÚ?æTˆ^o[?ÄzëKƅ"?ãs//š¦?ÉiAS»D?‡èl*?›g™c¶*@?ØZalÁc?È»Í~¬?Ûqˆpìœ?²îÜÞÔ'?¢­.èCø]?'š¦Ìí_é?áhØþÖ­?³LâH|û?æy¼_tã4?±'äÜ1E}?•-øhÁf?Š¶¡¶J^±?ѹ®`êÀB?°m÷YJMIXED4FGL J1702.2+2642¿åD
ŠúfÛ@A\‹ÁiÂ;À:"E>ÎqèÀ<ƒ:"ÀÅ@%|nWÌ@®M]€ä—?Àóîº2kb?¬±<Úý?íS?ˆÖÿ@	d\1"1}¿ïû>¤€?ïÿbì^bŒ¿ãrí]f¤¿áÌ@µÒµ¿ãˆpîèV¿ãÇ(žáŒAGNbllMG2 J170210+2643?ïöl†™•E?A» á[‰Ï?2£²ÀT?"0Äͽ}û?Lü
)¿™?=¦È&;?ïßÓJróp?n"_;?ApIÜ]?LýSôI©)?kУU§[?i5`n†™­?ïÅ7"H?lä\^0o?PÖS¹Y‹3?Sèþ"Çm?y.¨àŒ¯?j¤çS~]?ïµpW•Ç?[º»‹²\?b:¦¥é`?B²mp8±†?|*©?‹ß?YVGÝÜ?ïìàsu?Te±-1­÷?Dà%½6
ö?;6¤fŒèÂ?[ÎïrÜCø?PË)›:µ?¡ëD)?"tÝÜ6q?S…%¾Æ?`€Æ3âx?†#2ÍO¡?'M¤ç>1Ñ?Ý/'?sêÞâX¯?WÓm‰õÿ?NvF æf?"±ÃP â?r»ìnó?ï@):B?w9XV"_r?v#‰J0A?_°¶ÌôOŸ?'uÕtZ'»?u'Æ°lޔAGN4FGL J1702.6+3114¿ïü—kÓ@Aߓ‰µ À:R2#h»À<vòS4Z@ P‡[SÇ?üoøØ?¾Þsþªjw?³%ÏG{j?öh†>Þ@\'t/'?ïÿþBe«+¿ã¢UË
¯ì¿ÝþÄ+=›l¿Í¯u£ñp¿ÝÒõ:ªú¿âÁ<£AGNbll3FGL J1702.6+3116RX J1702.6+3115?í½ÝFJDÐ?½ƒO.«'û?eÊg\ò³?rx´f?±b'Ã-ë?¼ù©í­J¯?ïÃïõWÍ?uþ½Ø¹¥?Oß¦uÞ?Sd܁ØS/?zéRìÅf?qÞ?‡ûp?î6'ŸÉ?Ÿ§Ï±Þ©?cn9Ù¿sN?i°†æmñ?«f¬ïòÃ?ŸyÉ´XP"?ïƒéÈÊÎ?qÿêÚG•[?t:n'[Ë?RŽ%ëD?š ç7NyI?p¥Ft¦>œ?îá]Ëjw?¤¬¸r¸M?`%KŠ^:?]ô/f›Ò›? çÚ{S`å?¤>\
et?ï\>¥VÂ?Ž_ÕÿNË?a{FcŽà?fÞ·<þ?'Xîõ é?‹h¢,šz±?ìè`hÂÙ{?©×I§Ž°Ð?kB[¾I?n~9"¿ËÎ?·âì&Œå4?©êðÐnË?íBW–þ?Ž¥œâBb£?Š"a°Äåj?q¿ý^J›'?²š×Ù^?ŒeÙe\\AGN4FGL J1703.6-6213?Ǥnß±«ßÀ(â­ÄÉÉÀ8=֌i/oÀ;aª‡'§@G–¡—"Ý@áª$+Xs?¢þ\緊?ÃXeœ¼ä¢@Ê&½+.@Â*f…ðð?ïÿ«çy÷=¿áˆ¶‡¿åñ°F"HϿ婼'ì&.¿ë51ÛD^Õ¿ïÿø="ßEAGNfsrq3FGL J1703.6-6211MRC 1659-621?ïc< oK½?œuåSd'³?wƒæpŒ+?{סroñ?‹¯•é½œ¤?š<˜'LÌÂ?ïÄ£Tû§?¡e¾Éõo?eO±°rU?uÀ"|=s—?ŠºêÄ{çÏ? í±©×?탋måi?§	U>Jé]?®A¨ÀÔâ?¢r¿À>?¡–ˆ'íŠ?˜,÷³?ÿ?îéߒո·?†¯UUtI?…›]Hmr˜?sË*:Ý?—ö^ú2÷Ô?€
zü¼Û?ïÐRÏkõ?£˜®H÷A?ŒÅÀ"½[?˜±Ìà%Áœ?'Cf_(±?'¾¢"Ó"¢?îÓÆ9xÜ?¬Ûö>îÏÂ?…h›÷ø?žzjþqL®?šÓ6´èz?¥aÁ"˜)«?ëÑnüX'?¬ðB!&…?¶Ÿ3íp	?¨ÿàø+?¥ª¨c¯Õ?œ'¨mEH?ìªcðë:? Þ!C0Q?¡pQ@¢M?Œ Åœ³³?±÷d?K˜¥?šÄ½Ç'È—AGN4FGL J1704.1+7647¿á_ËWµQ9@@1éÍ³}À9@UÁF‡À<M¼¢³Ï@¬ÙIÝė@S°ÄXŠ?§ŒàŸ©?‡–!jŠ?Üî~Î<9@­ÿ±%§Y¿ÔȨZ§–\¿ä_ÕÑXM¿èO/]e¶¾¿ã_lÂK¥¿éï81Ÿµ=¿ïW–Š •AGNbcu3FGL J1704.0+7646NVSS J170357+764611?ïç:¯±çw?Žéj'þœ?Sþ4¨›£?|ºõŽéu?]Œl^ÉÌ)?€ü6.Ö¦A?ïáø"fo?qŠYÀO¸½?:ÛNŸå?FÒ·s¯7?j¬s£8R?püÑ=E?ï¦ÿ.…	Ñ?~* ÁñÇl?c–)^àk~?shW!bòÝ?Zª5üõ?wÎÐ:ÉN?ïü÷½;_R?"j»æ ¥?žà˜,7?
6;cÿé+?1\¥Áƒr?o­Ùœlƒ?ïíËÀՕ?[5|•#&™?PN±ÞÊG?RB3لÂ?U"PG›>?QRņœ¼?﬈ìo¡Æ?•ù͸f?JœÂûeäÛ?\_``Y†?ƒ3ø¾ŒÔú?•ºKsy|÷?ï\å|Ø)?†žO†±ý—?iý
v|j?t@qýûÆC?'#®¼Þ›–?"þ¾'" 2?ï÷Å"Ö¼?Bº*
Ï@í?6F½WhÿÝ?+z3ÕåR?EÈi‹X?<aڛ¸N¹AGN4FGL J1704.2+1234?ßò£ý
@=f°¦üX¬À:UÎyu6äÀ<E¢Ä»†S@'ê0µÕd@1wðÚÉ?Â#•ÜJÄ?µ(õÂå?ñK
¥uoï@
jŸHZ6Ø?îÔÎÞõÄ=¿êè±d'z¿Ö{%¥«ö"¿ä¤5~ç煿Ý@ˆ[XÁ7¿ïÿï0l¯AGNbll3FGL J1704.1+1234NVSS J170409+123421?ïÃÿRtÛ¹?«´(\²¶á?n>ºPúh™?«ÄÆ~`~?mÁó<éŽ{?f£Ÿ:Yv?ïܑª¦¡?izz7.5?A7w"v ?H%À=¿Žô?o wGHä¬?e­Õ(¤ƒ"?ï–0Ÿ…?Af£â@§?aˆÎÝ&˜ç?o©f¾†S?†-ã˜4?{¯¥àl?ï"}a_?dLò¤[?E?Zƒø;FBQ?;~Ý¡­G?ˆ¦á¦"«Ï?c‹Ùò`k?ï»<ÇþÔ?–|QýQ9?b9֕ïZ1?•ñLpâd?y`ö`'0¾?sAé\å0?ï kߐã?ƒ<ŠŽ¨"¡?R	8Y«÷y?[@FôˆŒ?…£áâôÊ?4ç•#¶?ï@I´T?ˆÒƒˆŸ?eA€òd|#?mxHì!a?•N™]bw?‡""fé\ê?î¾9	<?')ûÊcØl?qFKz
†?Z;ÁõÖÎ?¡ó¥u?vð?ú1+AGN4FGL J1704.5-0527¿æó°å¡Á@4ʂƒÓ^·À9Nµ×½Á—À;ΛâI5Ô@ =(Ɲ³°@Ga)Ä?®tÉUží쿕æ…ZZn?éά€§f@ý³¶P^'?Øø¾RW¿ã‹rX¿äÍhø¿Ûr£áq¿à×{ýQyð¿Í;;~AGNbll3FGL J1704.4-0528NVSS J170433-052839?ïìŒñfú?RjyôUÊ?9áÓÑœÀ?(Ägaa™S?`7©^»{±?Pdr"ËÀ:?ïÐ!€ü6?só¸Õç+2?N¹5§V]?Y¦ê&…>?t.7>P¸?o}{fÝÎ?ï¢`¼r%{?xÄJœ*Hv?]¢Zbíû?dD^f®.?ƒ³…žÿûÉ?t¨$Ææ³C?î܂afÛ?xÁÌû[)–?pÁhùê@i?MœOV×^•? ¬É›@Ã?wÀØy0Ÿ?ïÔH¤ÎE?k£~É!…?KHY^ƒú´?A†ÝÄ9‡À?rˆÐ£ºèp?hӛp¥ÙÀ?ïe,÷Ò+?Š¬Š`õ?\&¶I¾ë?eeäÓÚ(D?Œ¡ÞIÕ«?‡÷©ýçbT?ïY¢Ï‰|?‡
½Hn…?b¶É•á¯W?]£c³š«?'…òkïq¥?†.ò4Oå?ìÀ÷Ëf4?"Ãѯ ò?‰Z¦Œ¿Ã?oƒ"H"Ä?¶Ìò.j¨i?"'aøÔ¤AGN4FGL J1705.0+7134¿é[ÖQI¸u@@úˆ?Õ%À;%J<d4À<ÍB=Jä@úCºÚ1@‹Ó"Qc ?Ë
ær@U?¿œ{Ì)8Þ?ò±‡Ìè{@]Ȑ'*?ïÒ(ŒD¿Ý*qB¸a[¿ã'<"pj¿à@ÛÈRé¿éÿ-!¡:x¿ïõc#»ÆëAGNbll3FGL J1705.5+7134GB6 J1704+7138?ï°Mü??r¼á^š?\`Sv7%?Pß·%E?€`·'6–?oNãØ?ïÄð""V?s&Vr|Æ?Qh˜Ô"†?UÄ*©Ü9?y@£†qç?ox,×bs±?ïtÞ»Ú¸?}™:]MÕÍ?d°\Öÿ?aA ì±o?ÁäøxÞI?{Û$¶v?ïŽý–:¶Ø?cA&×Se7?ré"d½gª?N°)9Ò>ò?'ËØ/ÕN\?`øs"ƒL?ï+•ïYÙT?‹[û*7žî?s–µˆ·Æ?jtÑi1?•§Á!3[–?ˆuSn[
9?ïdùÄñ?‹FÉX&Ì?b©nس?g[vÍ*¯?' RRT­ú?ˆ&…Z/fï?îâPÞ®?<&™>?s]Ž~´?p$.'™™?žæ5Èqšã?Œ»QÎt"Ç?î͘šs¼Ä?~P$‡|?†Í¯™Õ?hô
{'±?šþØE̟?{oœ™¦AGN4FGL J1705.4+5436?澖iՏ@B~¹ÃÌîÀ:Õ3YɟòÀ<΂€x`d@ <–Þ(i×?üeћh¦³?ÈzxJB?ÀFí9Ô·þ?ö HZå?ÿ{=pxãì¿ëÇퟫ+'¿ÖŠmÂ%S÷¿Þ]*¸b2¿Òg"ÄËL¿åè4ÂTxÓ¿ÕpÏØAGNbllNVSS J170520+543700?ïÛÂ'n?`"±ê?Bd·ž5W—?2ü€s†ZÂ?p3Q?]ð¨_ŠH&?ï¶cê5=z?{•â'ÿÛ?Y½ï_)ùQ?a®¼P[³?~^Ep×?u]›îݯ?Áqò-?sƒÞ ¦ ?`t}bÑ»Z?\Û…)Œ?Š8ðW-Ï?q;òŽñ&¡?ïA¨+'º°?p!E@Å À?{Ì:÷éÙ=?[`Rp{@?×ëÚq4§?k֞¸Šq?ﻑ
ƒ÷?pÂ5SMÍ?TǭΘ¦?Jr¹Aò?}Õ‹xG?m³Í¢6)?ï}H'O"?"ñ6¯+¶™?n-¤&ùß?t ZDAh?™JµòB?'ÊX"g¨?ï)y©V°?€­Çö¯æ?h´§Õî?buƒ~"ó?—º5û¢hÄ?}‡("òá?îp¢Æ?‰"»êÒF?¶'h4#?u÷dÜt?¦«t<±ÄÛ?†®óe@`=AGN4FGL J1705.5-7423¿í-—ÛÜè¬À3jâ¸Ç\KÀ;ÏO?ÙÀ<Û÷@=ݱ@#oÄ8(»`?ùŽ­\Äüõ?Æ_šYÝìÛ¿¬6^ø?çÐ3:}ª@'¹Ëé"¿ïþƒþý¡¿î¨§ž¿ô!?ïý6âjBê¿âÏ@Î&i¿åFß•e?ù<a°@AGNbll1RXS J170548.1-742240?ïϕ,el?qþ‰þ?.M
ÅX?Îօ£v,?wEeâu?qÄM@µZË?ïyæ'‰(U? ÇÁssd?a¡¿á_‰†?mY:㼌"?~Ð}? `gœ¥?îþ0°T¤¦?');¯ûÓ?[¥yþr?^êmÎbï¦?ž'N¥E?'~ÛâL?í"b —¶Q?ž @3Ä!?^Þ#`©`?T^ÛG+ë?³avkmì€?ž4wen+?ï¦Ïÿÿv?}¨é ˲?<mhêl—?1>¤N€¾?…kì†RIa?}3°?îß²…MÝ.?­âûá'ÿ?nG±Õݐ?|ÖÖ,DF? ##,Á.R?«ô:IÞã~?îšcjLhÓ?'ëúÄ¿¨›?c%Üc½Ç{?i%£ár'?¥'kÞ]?'®yòךÓ?èjÒù%Š?·´Hè?paDb`jt?r–åJú$¡?ÍÑ©ø®ÊP?·,ðÖ,ÍAGN4FGL J1706.1+1000?ÊÅtFw@;åƒjƒ,À:?Ò?ÓT¦À<ãAƒX@¬åm¶@³@ÔÜeÇ?ÉȹAՍ?Ã
é!›?õf"X@ÙÛÃO˿ךLGo'¿ãZÛ¿è…tžtG¿ì3l>¼¿ïé!ACAH¿îÃøþ.ÂAGNbcu3FGL J1705.5+0948NVSS J170556+100006?ïð6¿áa?V5ÛU¸?8#ÆT
?.ÍrÆ~¥?Y‰–Ÿkü?T.~C^?ïÊ¢"0ã?x/lãÛ–?TÓÓhšæ?`Q¼àÄo?uz'؛ëä?qó«ÙA59?ï{N%õ*?ƒ ƒ†p­?eT(ò¢ª?e&v9—w?‹üruXì?b\:ð5?kh·W?ewG6®¾s?izd9?Ji5Æ'f?‡ñà¼õ'‰?b†a>Ä?ïßÜüð«ú?faˆÇiƒ?D)'N†°û?8µe•?k¹l7?eCÁƒDs?ïe[—v?#s'`ÿ¹?d]Šäæ
?nÒxn4ì?ÈëR²6?ŠZ]|Yƒ.?îú"©Ù"ì?EØVŒ·[?w‹6­Ð®?x‹Nߎ?šÌ 8Žû?‹"ò~ÉDé?î²ÃjÙ?…B8Cê?€
5ÿ0™E?klæÊÝ.? Û†RX× ?'i™ä§ÑAGN4FGL J1706.8+3004¿Ø"'Œ~p@ALSóÀ;9ï•N±À<¥o@Î&@ŠM<žÁÍ@SÒDÛÒ#?ÅLLfn¿¡_w½Yoæ?ÜóD›:ƒŠ@ûÎíäJ¿ï5/øOó?ïþ¨Fۆ¤¿ì¢ì^b‹æ¿Ðì±#yó¿äC‹ƒS?³!Þ:øAGNbll87GB 170454.3+300758?ïº÷œŸ?sWÈ»³†h?M0ÒnËA?A¬‰ït?~Þ^&UË?r›wñýS•?ïÛ¼(\7?lQHvH?BUGøW?JL¤µú?o®s‡ƒ½?g"ù¦)û?ïDfr‹õ?£[Þ»?eî'!jK?gjê®U?š¹®M_ù?Œæ"h/‰?ï¶2;2þQ?`Á*ü†ºv?]_û<-¬?DlÅE>"?}Žã¶/ëÃ?]‹ÅNc?ïßz"2ç?€"§úBlZ?aþu¤çgm?]¤Ö ¤Š?‡HƒêjHq?~qýÞ9Ÿ?}?…"'Æ,#é?WËZÊå[?eÏt'á5?‡–íJyS‡?'é# :c?Áu¼×?"둇G?pÍùû]ž·?qÓ;öÙI?¤="¥²åB?"àœ''J?ïIx³´½?~jpƘ~‡?v®9‰Bš?cü–Í
,"?–Ð%`¦w½?{;>ìðÉAGN4FGL J1706.9+4543¿ã«
-@Bo.ßç[ÄÀ:¯¤Z½»¸À<_8ö@*‰¹QÅÅ@Ö#£s7?Ëÿ.^b6?¶~³Ë?é½ F@iùY¿Û^Þ&'d¿è-ÝvV¿æÐ
>Vý¾¿ë!°9ï¿ï÷á&öå¿ïÿöµšAGNfsrq4C +45.34?ï÷;ÛÎGv?DâŒhù?*Áh¾Ðø»? âîh	?L`6NÒ÷?Bí7gÄÿw?ïÉKñΗ†?y¨$½ŸÁ?T§wÝ@J?cÒè¾oÎ?v0)@Pµ?q—"‰?ï©(BòÌn?q ªnûΪ?[ƽ/s$®?\šHµ`S?'=¨µ5Â?oіñؤ¹?ïۜíÐÂ?Y{ôV0ü?\j¤ŸN?Aa@ÇÑQu?wˆfÒ+5?V¶Exçf¼?ïé'…žK?`lWíSâJ?7›©Ë­k•?3÷$¾Êä?cåq3sõÆ?^Ÿ²a}?ïcŽ€izv?µ¸v8?ao/¹ZAþ?o;ý.Ûßá?'`Iü)Z?Ös
p?ïNlÉyS?ƒIώìj?g ‰œÓ39?e|AÄAu-?"KÁ*ŸiQ?'ðë·1ÿ?ïGSZ(?|vV'®€?sÊZÿmo'?aö Ô{?'+~×ù"?yšj–v~AGN4FGL J1707.1-1931¿ïދê4Ö@(ü)¥ë·À:ŽEîÑÀ<.·~†îœ@éûéd2@,p¼*¾?Êdk9‰äp?Øà۞KÛ@¥þ9Vbã@Õýê&$¿ï¿,Ñ?ïþÛ<Òf¿Þõt,öƒ¿á‹B=è¿ï›Ð`U*T¿ïÊ1¢ˆ.AGNbllPMN J1706-1932?ڙ`ÅxÖ½?Älõقà?Õ{WÑÅ|n?ÄÜèìƚâ?Ï֎Ï]˜.?½ÀW•àsë?ßeY¨ ü?ÉOQT?ÕÓ¾œ§?Åh€5ß#Ö?ōÑËup?¿¾¹ëëî?âÝ}ôøe?³âNôÚ²é?Íô'Ä=\,?°eÈè¢?ɏ÷CîÂ@?«z$…ܨ?áßP"åLB?¥ÔÛÈlÿ?ÍMÏãúÞ%?£1À8/.?Ë4íÈoðÔ?¡Ù‹£Áù{?Ё—«i?¾³dú^3?ܑˆÊO«?Æéó@ÿÐ?ÓUõžëÖ?Âu‡B,?Ô
üyÛÀ?Ç^—´€êe?Ýe#kM?Êëî¨66ë?Ϳb?Ãò"½®ï?Ø»«Bʑ?·)vØ	Òù?ÖsYF ×?¸ßQ)€ft?Ñ8ácîÎ?³!t²¯Ç?ÒpáÆüJ¶?§¢2"|Ô?ÖâuFA¸?°¢í˜ÆÌ2?Ö¬¨òts'?¯£ËóDA	MIXED4FGL J1707.5+1649?íø¡ž?N@>VÌ¢Ûa»À:4¿û-2À<L¡3ß@üÀ'a@DZ¢ãÅ7?¾¬W ùå?¾·ñH'$Þ@f´A»Œ3@
Ž~ZÎؖ?ïÿÔač¿âá',"³¿àêŽ^}
ó¿áŸv¼Ï)¿ë5â)>¿ßÙÙ«Ø`AGNfsrqMG1 J170732+1649?ïÝoLnjz?eøE"~\?I0xép>î?Dµ.ÇîL?lD•]¼?c UþÒá?ïË:räñS?vfϷ̬4?VAÉ]0yœ?_
ž{?tÒT®"'?oøv¨a¶9?ï8´çJHñ?
q`HØ?xõã!À?Ê¡Ô›/?'«êUÔë?ˆø«"eNÄ?ït´|¸b?f ›ÞÏâ?wŸÉšLvÃ?T·M2Z"¥?‡
Ä?`oª(& ?ï³³œá2ò?wƒˆ£æ™?eûÅ+ðS?c{½§÷?{™3¼žÃ?r›"Ì¥gˆ?ïo7¶¬O?Ž·U¥³?j­}Eã?tšßêÖ ?±[´¶?ˆ‡½æ?îëúYDaP?'É۟±2S?'~ý§"?'¿ ¥À"?šœs¼ÛÖ?Žžöˆ"‰Â?]¿4?'$g¥˜
ç?Žƒi-Jxæ?q"¢3¢?ŸJ?ª•s?|&ÂFÁò]AGN4FGL J1707.9+0016¿ÒïÙ
!ü@6ü{þ~ÁÀ;‰‰¢À<D]­Z@¾@ Åå،s–@´ßbцp?Æy§¡D2࿔è:D')î?Бz{Ç »@þ=ìʙ?âziR©ñ¿Ø'-¿€Þã¿ëÁ
Áú᳿˗)gW}¿âòÅ_E4è¿Öi:@ԕAGNbcuNVSS J170744+001750?ïÞðá݈º?céÍÓ8Ø?1p|aB?& Hb"†^?nátvBQ?cMºû¡É?ïÓT•v?tm0‡Â¹œ?@øKCòn?Ià¼?t6¬ ?<?rp:jÆX?ïa)øÄCß?ˆb©6}g?WÊۘ.ÿ?][¢$Æö?'^&e~ç?‡®Iʑm­?ïŸÖ­ÿ¶?h)ðj7?AèZ½Ä=@?(œM¿D2?‡D°ÑG?h:é[H?ïдI·ó¼?r——·p\ó?8І¥å…?0t ë}Ä?vÒ©lŠÂ?rþ+]Š?ï•ÞivM?ˆÊ'R+¶?P"0Îê=?_™‹)-é¥?ˆu߬أ‹?‡#Ï{ÀÐ?îސ¡£SW?'o˳Õ×y?b/u›.
}?fˆ¥»›ä? óþ5Ék?'	ã(Þ]?°®"?ˆ•oŠÉ¿t?_GLII•?PÄ˟nÑ_?¤[ªŽž
Ô?ˆdö58AGN4FGL J1709.0-3525?}'¼59ð@ŽÆ±À9ºâP3À;wjš¨@uZê²@f'amÙ!?ÑiIºß™?׺@Ù$@Y¾L×I(?ûÉTZ[:?ïß(Ÿ[zz¿æI]Áý¿ãù±œÅž¿çޘÜÛ7Ê¿êMDƒ½¿æóï»åüAGNbcuTXS 1705-353?Ð}>¹=È?Á«þ/49Ý? Ê$8NÁ?"ŒW¤&ï?æ´¾b¶à?Áéò†‰‹H?Ù¹RÌևâ?Ä{aþ«IÎ?·]ûñ+ž?°fZŒo[?à7—%?ÂÚPƒ{0?ÕjcµuÜë?²_­ü²U™?½}î9ÑTh?§	e·m€?á›^"W]?³'ÀÙt\?Ë;DãÏÑ?™Â¾
é¸ñ?½¶¸ÁÜ?'ˆñÉkZ?吋ãoóÐ?žÌ÷ò?ÁJR'&¼5?°\î)ª"?£/ )"Š?˜çÆ.ÿL?êzyRs·ª?²Ûʅc›u?¡6óÿc?¼*/,Ø?짛îf-?ÀA‡×Ó?ælˆ\®?Â]®€uJ?ÅO¹³Œ×6?¤å+Ÿ]V\?¾ñ5HŠ‹?©ßE^ÿ Ò?æÍêê8á?±ÁÂ>¿³~?°8Lcæe?Š†tž™zé?Àˆ1z©òá?ŸñÈx·ô9?éÖêº;? ƒcÂàjOTHER4FGL J1709.7+4318?ç÷LÔ*Jh@BÆâ¨eÀ8dVôÙ[À;ÑLF)¯ý@¶Ò«@Å}?Æ¿m? µ"â>?¸¦‹€¸]e@ŸAò×s@nE­ß â?ï¡Ä«–`¿ß!æúËb¿¿åƒC…¶ä¿äÓkL4"¿ér†áa¯¿çƒÐ¸ò$AGNfsrq3FGL J1709.6+4318B3 1708+433?ï»L{ûñJ?­y¾#dÿ¡?]w¸û)Ý?RðU>&%Œ?zûÔ&Øv?­ƒºµù·?ïÑÛfm?v|P€œ'¸?J¼0¹• î?ZŸ2†#?t%O~ÎS?t$TÞª ø?ïqß(€8?<‰é»T†?sJƒ1§Z¶?Ö5	®ËÌ?Š–…­?ŠÏW˜Æ ?ïúâ/›µ9?,踩!"?%ò˜Ù	z*?©‹eAÞ?=õ8i9'»?'uË'?ï°¤ÇsÄ?|{4ÐÃ-?^ÚSë:'?R!H§r ?÷žÝãº?zå?€ô¯?ï…g𡊡?]‡.Wã?YÓ鈶?hŽïZՇ?‹k£O‹?Ž˜õ+|
?ï{}ž?"‰z÷ôÁÿ?z¬\EwlÂ?'¥zÛ/¿?–bلH?'2œrW"x?ïó?èÑ°?Iý<VGŠX?:vv™üs?1ŒoëÏ<?Râ'YzïÜ?E²z Õ8AGN4FGL J1710.1-2030¿ì5»Ùèò¦@&°Z-rÿÒÀ:¥P¥4À<(äSÒ,@bBÁñ@ÐAÌS*?Ëü¨>O?×éw}e"@o?Rü&W@M™¢Rû¥?ïû´a"ñ¿åd8>4îõ¿ÈFû&§^©¿çŽâá·ª¿æ÷mT—1
¿ïÿW~lªAGNbcu1FGL J1709.8-2026TXS 1707-204?엻RHn¦?¯*–dW"?' 6'tr?Œ!'ܬ­Œ?¶ºÊiH®?«‡«6xWÃ?èŠ$ÊBa'?ő[ÌH\T?±ŠõaÍl³?±õõÛ¦éÀ?Åò%¡Ð?ÂLŸ32?ëËÀQƒ>?£¶G¦+?§¯âÎoMæ?˜«P'(ò?µÊA››?žË¸w@®e?åTÑj/7•?£&è͆â?·GÇïâ3c?"`½`òSÝ?ÏÖ_¿û{?¢Ö_Xç3?箽9©;p?»Iæ_è?f?©0¦Ûj?¢Æ±Ôɧq?ÊøápÑVþ?¸(ì®û'Â?ßÖïn?ÐÁ,ýÜ\?Ç}ÀjhԀ?ē
ûF¢?Õ*HÚJŸó?Ìy–ëzž?èibe–¼?­)>]uá_?³¼]GK?¡'€Ä¬/?Ä|G䛬?¦þ-dŽ¶?Õ=ûAîü'?©Òè—D?ÅÈ ž[?©)áÌp?ßÝú­ÁÕß?°#U	Ó°šMIXED4FGL J1710.3-3943?ÁødçF†Þ?¦Bî"n%3À8@‹áJÀ9îÐè»?Ý@ܶlŽ@Ásûz_B?ºÉ³<ØÎc?Òê©â<Á@¶8ݗl@–f‹û r?ï¯Çˆp|?€œ ½­Ó–¿â‡ÐCyÒ¿èöN¦V@¿ïi˜¾&A¿ðAGNbcuGPSR 347.050+0.041?Žhe¬óŒ¬?°‡"ÇËÉ?Ùw¤š\?Ð?ÌM-
á@³?âʌGM5?ÌXÔ,'…(?6ï¿æÁ]?ß¬¾q?×ÄOÜrml?¼ï€&e?ã4 "'ÈO?½œ(÷èPÙ?ªñƒ\Á)?ž•À•2¶ô?à•jõ02?¸húú¹m?Ûvùª&Ú?·š¤!'¾?Ž$€bŒ?t/8zao?Çhà"Xß.?£Òä9·?é­7?g?¥4·O´Š?AF¾—à?uùª—>Ä?äÝäïzÄ?Ç°ªâÙ?×j:ŠX‰?ǔ­Ìxf?‡.‡V÷­?‹DRÇ †?ÖøUɂŒÚ?Ã_¬Ÿ?ä'ÿ	àÔ?Ãå(8Xa?›œ}oYŽ™?'çµRÕz?áýؤWžß?»`1R?ÚJ†àÉÙ?º"´c…œž?q§÷AÔt?`7Æ-]?ͯbÜ»?²AðFÙÁ?èp׍3ôh?²€¾/ïëMIXED4FGL J1711.1-4600c¿íEýœÅÞÀIZ¼äø=À9œR3©z¸À:µs¯ûî@ÿö¿ºj @i½@gÏ?ךŒàŸ?םŸQ>Œ@ÇOšr®@®ÞzIG¿à7(áÀ?ïÿÕ"[ʁ¿ê­ÂC±Ü¿èV° Ï/¿ïîõÁ2e?ï
•ö]AGNbcuAT20G J171106-4552548?áÂФj$ƒ?Ê´~¦'ë?Æ
öló?ÅDaȋ¹K?ÑyY;õ=s?ÉZTâQæŸ?ÕñÇ°$ÂÏ?ÈS؞€øÓ?±!Vò0?°`2­ÞC?ââñIXäs?Æ›eE™?×qãJpD>?µ°Hó¼?Æâg^?°À]l†€?Ý鞍}?´žM*d´^?ÄΦó«?¤)ïé Y?ÁWw'€?¥¸#[DŒ[?æv%㥓?®bI³ý?Ù·©,½+?È/,çaé?Îêh·³?ÈýdÃλ?×UÍfü?Ë3ºnȬú?½«bދT÷?»ü™}ü?ºy<abÏ?º¢ü"J|ü?èûqÜ¢i?Áá\ö>úÖ?Ê׏Éa2u?¯ÄL¸¤Óˆ?ÍV–om¡?³{^@ä1ÿ?áôvqÌK?µ¥Y8:
?¢Zz¯OŒ¦?Ž:s­òx?Ä<2]Ô?´æhLi?éËQHáµ?µe7õI=MIXED4FGL J1711.6-5027?åF/À¶#À؏>ÕÀ9Z`ȗ³æÀ;mcr–'@BDmÃ'@WS£ìó?º S7
?³'T®ƒ
·?øÂ+‰Æ@t&µ÷HK?µëî>ü-ý¿Û2¼`¦¿ê©ãÉh">¿â'¾@—õ«¿îo݈†Í?Áê}ø(p7AGNbcu3FGL J1711.5-5029PMN J1711-5028?é$ŽËñkÏ?¾1CfS"?éӕT?¼?wdÂzÍ÷P?Ênv2êÁˆ?½˜¸2¶á~?êÐk?¼`Ø¡±?{÷§ù"%"?7š½ÝN?Ç"oM?»«XˆØ+P?ì2R£o?¥8"{d¨¶?™½Ø˜Püï?" Éîùñ?¸aÁsM?¡c3>w"?ím%Ûõ?ˆïùµS­?Jj~à?j7À¥eïb?°òççÐ÷8?†Sž#‰K?âú!üÿðf?ÂSÝW‰~Ä?"ÞgÏ©a?ˆÈ£ãË?ØÍՉ<‡Î?Â'ÇYÆDó?âëqþ†??Éɞx?Š¿dÚJ8Þ?"='Lïô?ÙSáõº?ÈØ={-X?æhþ›Ý¡?³?'D·?¬ÚÉäµØ²? E]åàÛR?Ï%SHŽ?°R6"`?èïSª¡ÿš?¢=mŠ!J‹?§He|4°?‹]{'Ùf?Æp—ö4î?Ÿßë>{0AGN4FGL J1712.5-3142¿Ô#ÓM‰9"@«½À9ÁöBçÜÀ;2H˜F@®Ÿ]'ùC@be+ÓÃ?Ñ|Òì™q?ØѡȽ@²q¼Û¾?þœyGêz?îÄ!ÝËLÅ¿ÔfˆË<¨¿ê§(-E³h¿å¼þùoÿç‹5ó×ӑ¿ïÿõ^'AGNbcuNVSS J171309-313912?ãªÍüwµC?Âí¬…z~?§ï3àj;?¡î8ÅRáÎ?Õ¬}‹_ÞÒ?Âm•ðÓ×?ÙçÝ/¬§?ù{›E¯ü?¼ø›˜Þnò?µŸô)Až¯?ß¾ñ<˜·œ?Á'0˜	‡Ï?ß½lóÛ?²túôØxŠ?ÀA½$8C"?¨cøGÛÓÿ?ØÇd3?°ÃµúÊÍH?ÔDø¶T?¡†×cöí?ÄÜ×7p÷?œ
÷Tà¬þ?à¼'µÈñ˜?¢:šëD?׫Ëâä]°?ÄɯG<?Â+é23.?½†ÎÑ3ä´?ß>?"Q?ÅÜ­­J¡?Áïe†  O?¶(ê\!5|?Ëó·/µ,ü?›9®ï¹ƒ?ä‡8Òj¬­?ÂÀRZ°?ÑCK™±lt?®@x"	à5?ÇónRª-!?²‹»Å\xÎ?áa~óN?²­A?üŸ?¸»×–†=?"ÓŠ‰¹Û6?Íá§kO•{?¬ÿ¯'íA¦?åuž©½—ê?¬—å•iµÜMIXED4FGL J1712.7+2932¿Äøà¤Î‰™@@t`$-À:HOžÀ<e$îÌÑÕ@ ˜V]¯³Œ?ümfL~?½
ãÉ­?ª$÷A{±?𨯠Ä?õeª^Ôê¿ÚIËÛ¶µ¿áh¼""Õ¿àXa@ß¿Þ~+ÿã$¨¿ÉI"ƒ\ì?¿Ú6›¦AGNbll3FGL J1712.6+2932RX J1712.8+2931?ïožú4A¯?œNŸ("m?gŸqñÜ?›r úc˜]?Ž0ZET?5@û?ï`¯°åÄ?'%¬"OR?qV}ÙnÇ?u
"àËÈó?(Õ>éÓK?‹Ã+•¥¬?ï(;÷Ž'²?†‡	U0Œy?ruóÐÞ[–?tOd9¸úÝ?–[?1á?'}ÍB	?í—É]#?‡È€•oF?…ñAȸ›1?lŸh=fŸë?°‰1}I®?†³~dbiÒ?îô"#ãßä?'LÇ#­"¨?i¥·8«¸?cM¾÷7‰£?ž8ĜƂ'?Tvðdf
?îU9
Ekx?¥¥?rº?ƒÜQ6ÂÌ?‹ß[ßhŸ•?¥ëøi³T?¡"AVZ¬S?îNëyFy?•¤¦ïÁº?{[‰ØJH?z Šv&}?§œø7£t?"›L¾å?é Á¹üÄ?¢òÇ­/ ö?™Ÿ'{!?‡©ÇbuX+?ÆLÅ&Kl?¢˜À³g_°AGN4FGL J1713.7+8844¿ä1»iM š@;¤ß&k¤"À;Œ`b@føÀ<ìXJCðñ@!aTБÓR?ûNB¸â4=?Ðë}&œKü?Å4á^)V?öžÜd…@Ó~Ì
à¿ïÿÔÌuŽø?ïÿ®XëT¿ÅZF@+>¿¹\èä/"î¿áŠ!¡»Q$¿à…ïbùÊ\AGNbcu3FGL J1711.6+8846NVSS J171602+884416?ïè>cµ?[-Q™f4?AÔSMØç¸?2›C¨ˆõÄ?cL‡å¶s?XU?eIÊ?ïÒLþáG?q¼ý\n¹D?IĚ?ˆ?Q£¤9L©.?s íS0¥Î?m]Š Š!?ïm‰ç†Ë?~j-«wÂ?djØÎ$F?jÝJ¿q?'Ïè0©?yâÂ*Òÿ{?ïeضSÓV?oL"?jþ×›r0?L±h>bF€?Ê—†#?mc¢Hã_?ïÚý²ÑV¨?a²šØò?Nµìd{¥—?AÀ01ÆKÌ?mTÒNpÃ8?]—Ø#!†?ï~£iQ'e?
ÎF;Ñý?[W/<Ÿ¸?dö˜Ä ǜ?Œì?ÏeèÄ?ŠµW/ÿ±'?ï	¹ûõëe?"ŽO
?¤$?iyÁn.?i§Ì‰ÇCÀ?›™ˆJég ?ƒ¥–Øj)?înGäE9p?ˆý(¿yÊ?zÞ±yPÎ ?iU¯XÎpa?¥¿«Š´ƒ¾?‡"4`ƒ[AGN4FGL J1714.0-2029¿ïò½¢ÀèF@%4f+®´À:N{.t‡'À<
-€kË@#ÿåSƒ?ùµ(Ö¸ÞÙ?¾è(råЪ?Žtøì³?Òñ£[dT¾@	¼IGǕ¿ïÌR>[î?ïýð@o[Ø?¡K'_¯ª¿Û¼J~Sm¿ÑMR-Ê=¦¿Ê÷µP-ëAGNbcu3FGL J1714.1-20291RXS J171405.2-202747?ïÌÑKÙë?´¦ø-3ü?P®âÞ1{/?c*¿ñmþ"?w¬i<ö?´.'FFE?îºÞÖÃ#^?±#ÊD?RÔz´²¿Ò?g:6ˆ®_?£»nÀ!ú™?±—høù?íH؁¿eå?£`Ðe¸µv?]V¥í$²?h¾M"w?µCáXÚh•?£EÁ>j?îÀÉÄY¶«?ƒÞð½Ï"L?VC
`80?A,|Z¹P?£AKU½Ž?ƒ×ÖÎÿ½?î¢i"Sk?«Fï&7d?cË9¨Ûêl?rÚ4|à¯?¤œ´¥ó²?ª5³ˆàô?íqBќüa?¼Hiï:"'?f±¸-BØ?ƒ3îDmφ?³ÀaSˆçe?»v{|^\?뉱¥\£ø?¨ÆØþn?f!ŽzÁ?q%ög°}?Á€³0eðÂ?¨Ì7‡¨A?ì®T°A·ì?T©ËLu?hàô†ÙO?\Gwxˆƒ?¹ÆRÛÖ;G?{´—¦ï%AGN4FGL J1715.0+2616¿Ðªb® @?×a»úìÀ;ú61ëÀ<uÌÆ폻@÷ݜ¨Ã@y'½µÕ?̳€u†>ô?¦6ÌoÚ®b?ÔÏí~<Q@j#¹?£R~ÁÀÃï¿ä±À¢¿äþh›Œ¹¿â-t½l1¬¿ïþ*½ÃÅg?ïæ?šIÂÂAGNbcuMG2 J171454+2614?ï¼3ŠFŒ?x~…É…~?`tÐÏuOŒ?Rœ˜ùŸâ^?y«Ò_='/?v¿5Â%>?ïzŚŧ?Tâ—ii?mn~?tår~VUû?‰òú©¸?…ZGXµ÷ê?ïJ:F?'õ÷0(2?pj$¬ŸÀ+?j`i•Ñ~.?'¤o}¿³?€ ,"‹M^?è­(?hÀèҌ¶O?_Ô@@Zø?D
¡.y?‡œ=ÔEä?fmN4øk?ï[-¿´i?ŒFu º!?t…I7¾ª?i¼äŒ¶?ŽüP
­"X?‰ÅrÐÇ?îÜ'QcÜ?ŸÚƒž'˜?t0'>èe?(0i?ŸtÉ«…)u?›REÿº?ît?º'G?"Ý˃
î?~äQüžy?xctA7?¤â±ÂX B?'¥¯p~>á?îum\ú¬Ú?Œ@VÛy¦?x±i…î?gÑ;	«üN?¥'ý
ÖY?‰³ˆMÙâAGN4FGL J1715.4-4025?ÁÕ­Pۏ³¿ò"ãw3=DÀ9Øc—À:ð}e†l–@ x>fB)E@ð	yü?À¦Th-á?·vÀіá?ø ­Ú™>*@jÆ?ïþü—åº?íØ@|g°¿å†\Û£)e¿Û‡ôU§ÒB¿å"i£ÙŽ¿é»ÃŽAGNbcu3FGL J1715.4-4028PMN J1715-4025?äÀd¥è»?ÆE ²›?l=1–RuÄ?vüœEââŠ?ÖF½¹þ?Æ*?Rb?àcW7kÉt?Ñ[ğµE$?€°5bC?‰»,°DþM?޳Иo‰6?Ñ©¨÷?ä€Ù]5ä?¶.͑c'@?š‡ý<6?'ÃHƒkH½?ÕUÍv×?µ.™z@â?ä¨g¾¼O?§¤BhP
™? l'èd?~AáØg× ?Ô¬ïÀå?§øðš?Þø‹O‡…N?ÄÃQùÇכ?q»Ý›7¶?q‰3ª°Lù?à`Bœ¡z¨?Ä×p:‹ÓD?ÕÆⱪK\?ÊõàP|(?‹x$aÚ?¦`œ»Ìš.?ä®®†Ý³?Ê ¸S?àJ«Û÷ž?¶ñ£û˜`?¡Ë€^™šD?"×5A¼t ?ݟúœ=ã»?¶—³ü¡p?Ú¯²KþA?²&¡­Î՝?¬Wó*æ{?'éº0w?àãG™"?²lþÃÛ[MIXED4FGL J1715.8+2151?íÎGfÿ@>HèÙrÍ}À;!•¥ïrÀ<Ž*pìÒ&@ó}Ë$@–U&£ø?ÍÕLù	ð?²8ÀxÅR?ã1&¹@(@"Üç÷öq¿ÆU±7pÉ¿æm¢À^ÕM¿à¶8 WäC¿èRˆÎp:û¿Í÷¤¼¸W ¿ï÷ÔCédAGNfsrqB2 1714+21?綾-‡?z¿*¨˜5§?Kk
?+Ç?@$ÇÉ3?"ã"íœD?y¹ê"ò>?ïš\j9.Ë?"ºì"W)K?a7ÂåœjB?et?´C?…ô¾|~¶?HÓ¼&Î?ïOOSO]`?|ùƒ‰‡µ?hãÙ½ÐÍd?YÆX¡ä
?'ùšc­ŸA?yÃ@Î{Ÿp?ïw;'jÊq?läÍÜ®¢ƒ?X˜¥™PJP?C~F
©‰J?!u'öŠ?kÙ_bª.é?ï3¦Rº?ŽáùÛ/?aéö«¦ã?v¢.(]rq?—Möڜ¬?Œv[&j?ïÄåðÑ?—ŽñK¼~ç?lÖ)"}¶?zRÑQT?šžOB-?"ª@µŽ³?î"mK™Î?æ÷5þ…?uÒ^^;"å?nCç#ýÄ?¤ßwçp§?Žô¶y7õ?îX€ˆM?‹TÖq]³?m©žU0U(?b¤=F
~¹?¨£ÞŒß?‹´++¬öAGN4FGL J1716.1+6836?ÓkZšð@@áOKD¢À9°›±¡ÎÀ<qD…kl@$´o#@ðçä€G¹?°Od´Ëy?‡Ç8ä"(õ?ÕòoÀ@X%åí°?¼]ø®§ó¤¿â'f$!Gx¿ç2bo¶Ç¿álÁŸG.¿è7®ø¦ok¿áº>À//˜AGNfsrq3FGL J1715.7+6837S4 1716+68?ïöÁ:Gy'?EÎ%ø5÷?*Rê[gÍÄ?Ä㡐Ò?Nf\"'4¦?C~°[ò†?ïåúeŒKÓ?kþ$Ӈó?9e÷Á¬¿—?F§Íþ+R!?fØÛAèTS?gè?Õ½3?ïÀt.¦¹?n=ûà¡ðõ?Sښ€¢?Z¯"ñýœ?zÏB-,!?j­e	Ó?ïømQ½?0q}¼õ@?3Šê

?.Û0…P\?D…CYügx?+W€	ǟQ?ïí'*+Ä÷?Tƒ"îNi?8PÅRÅÃé?+rÝ!>£.?^ÉzdÏ}K?R­õ¤ºè|?ï­ÐÕÐ?"×â¡ít?Nž•Ç‹^x?\[*¯"JU?'¢aûc?ƒRâb¤§¢?ï}êÅ
ï?yÔAvE?_–hšoÄ?Xâ4"–N?ˆ½'ñh=?w…ôW÷~ú?ïêsÞÿÝ?Qœ0wQO?N—á¿•?:%ƒ|á¥?[̾k'nÃ?K?³8¡ÅáAGN4FGL J1716.3-3421?ïhʋ\ž@ݨ!ò™À9X™I—À:½r`o¬`@ZO+â1@¶Ú@¨?Ä'îÆò˜8?ÎÅ3æ·Yž@v§&J@¥Xz—?ïԋ/Ÿ*¿çÇb\«¿ÙÏ QC¿r¿å\½p8w@¿éÄ
¼¤¡¿ïý"#–]AGNbcuTXS 1713-342?À!à㸪4?´$uâ!¡$?¥ÑwÆÿæý?¢œI±«²l?êšpJ¯•s?¹7gÜݳ?ÚÛðk¸_Ø?ŸâCEhÚ?±="/†Ý?¥-P›#•?àje÷«¨?ÅÂýfÙº?×ÌyéÇ?²ÔÔ±õ:g?ºt¸±e?£Ë~)aß?àñ'­U|?²(ìåj?Ó:ÐÂ6*?¤åÖÐZ¸?­üʈ¨DR?‰*½».a4?ä'Êö'tæ?¥ÇÜ r~\?»FDÕ>'¿?°DÄ䢶·?°~Å̶#?¨ª\*:u¤?ê"GŒu]"?¶½ÜX«Éº?ÆÕý€Q?¾æ›/ï:?¸®ƒ
µ™?¶ÞlìÄ7H?çeúUú'	?ÃÊ_6h¿)?ËCàÑ!×Q?¬ËÿÔSWU?½	ws»á?¤4§ßNüà?åØܶµð?°PL_¡s?¾S
'ÔŸï?œ«I$Ü?´áŒ›.?–À"~»ƒ?é™}ý±Ç
?£»Rë¤;OTHER4FGL J1716.3+3434?¡˜ÙA0i@@Òb^™éKÀ;·ÀÌ
Š,À=yÚ6AÛm@[ N@†A­
ë?Ó¡Fnªƒ?ïþ@_‰Ó@9¥e¶š?þïΔ£º¿ïëiÀú)?ïÿæ4|ßO¿Ïàœøɪٿì¬Ù¢s1ü¿éæràÈ,T¿ïVqáÄ«–AGNbcuFIRST J171642.1+343856?Ӗ,ËÉ~?È_Cqï±~?ã‹&ŸÚƒø?ËZPΤ"H?µNÑËË?°ýlIKÅÉ?Ì2Z_
ì?ÈO|"ûû?æ7h³-ûw?ɏîC®Å??¶U°ö'p?¨9w˱Ç?Øb9•í?´wŠuñ;?ß< €Fs?¶‡3Lžï?ÀÃM§Ó™?¥ãPê»T?Ùõ´Þª¬?°ïÅwÓR ?âŸìÔv†¼?°åR…¬ÿ\?›ó
!Œ¯¶?l…J"]Q?É7+Áµþ?Ã:r'(Ž¿?æÓë]VŽ?ǛBöÖ?¶òM–µp?±›••è"ð?¼ÌÖ²Ô©?ÃÃ+²Ð=?é'F5Òî?ÇQÈ&)'?¶ ÷ŸZå?¯×¶Þï|4?Îôû›áë?´Sj3›%?äXrx)?¹x_Ÿ8D3?¿U¦XLzà?¨n+š¢(?ÂtºmŠÙ?©½·ú
{7?éæ
r{¿á?¯§ŠSB¬ª?§Ì?Íz?›ãA®K,yPSR4FGL J1716.6-6707¿ÛªÅ0KLZÀ0Q€¡{kÀ;<MI^ïÀ<|ók@•±êk@<î?äž?Í/d\ m? j‹Üdî?Ö²Üá—à?þÌmŽÎºc¿ÒFr©jÈ¿ãIÒ±é¿èg
À²ã¿Ä˜†t¿ì!€ƒH¿ïÿîÝÃÀ	AGNbcuPKS 1711-670?ï^.'…'?ŠâJ+€?^ï{­[?Sy‡Á°?'K7ñ9çÎ?‰«ðóÃg»?ï¡:à{«G?†;¹6|<?[R•ŒaRK?aœ¼ ¯'?"Fõ5cé?"—Ú@—?ï%aÀÜ ø?lTÈ÷X¦?r¹àEÙ^?wKCËà×Y?–ÏpM÷®?Š×4:âW?îèqf}@%?{ÇOh ?qt8M"±@?W§>Û£x?ž"Å?z°™¨l¢?îóÇ5ð8?"Ð	Œ("_?elŒ?ÈÓ¨?Y—Y˜V?žÙ‡µrð?"ƒŽÁÐ?îÿ'¼)ÞÃ?¡¯ªÛ"í'?n÷¾
7̀?{€ÜaÔ×?œ0°³!ç? ï‡!qê©?î¡#Îç.M?"}Øœ	?v8+$yç?xr9FˆP¢?£&½¬cïÀ?'ñ‹æ+,N?ìЧû地?˜¬G_ÿ³Ä?ˆ-1ËÛßZ?u}Ì}Uè?¶uåŸÐ—?˜6ªèʤìAGN4FGL J1717.3-6045¿íòM²1ãÀ)ížbV6mÀ:ïdDM6êÀ<•—rwí@6ƒºŠ*@mUhƓ?ːЇÂV§?ܚoÂۇP@=TT+
@jŒ¢:R¿ïð‹ž.SÐ?ïÂ{ƒ€¿ÖŸ§z­Æ!¿æ=í¡X«¿íĜý|B¿ïÿü¿ÙŸCAGNbcuPMN J1716-6045?ìƃé?Zo?¨<P™Cµ?©Âªj9i4?Ÿ'ÓfJàð?©ÕõÛ?™ïàðg¨þ?ìˆró<£?²ƒ58¢Ý?¬i1?ýb?©šX;˜kù?«ŸÆ‰…³?¦qÄÅ?°\?é¬7¶¥™?®p†MRq?·J¦/hÉ#?¢4ÓTýèŒ?»SœŽ‡Ô?¤}Ö·µ£
?ê¹\ñ??–pÅ(ØU0?´TØëÜ5	?m$ãØÕ?µâ"-ÅÓ?ŽŽPsž/?ê®4´p=2?²Ï`R¤É?¸ÒŒ/ëË?¬±5…²'?±»Î.V ?¡b61é|É?è)´Çroß?ÅzŽ`_?™ö"O?5½¯¬?º­%ۏeí?¶"족ô?æy'%UF{?´teùë?ÂJE&-?­'Ã<…`_?Ä_ e¿ç?«pÉ+WœŸ?åó"vøZ?©9ku]¾ç?ÃÎåzÌ?¤7Ë+3 Æ?Ènep>£Ì?£oð¾CAGN4FGL J1717.5-8114¿é]B;eÀ7^'¸#È\À:–@
²
ªÀ<iqDæ¹Þ@×`]bÝ@ÈCæߞ?À»¡VQp`?Ž¥vLJ"?Ììa<°à]@íBDH.m¿é
Ï@Åm¿Ù́»¬i¿ä I·¿à^^…¿áü¦¯+Ò¿ã!R•Ï	¾AGNbll3FGL J1716.7-81121RXS J171712.6-811501?ïÝVf'Úª?Yö™=?D²ѐF?>ƒF4>?m£ì­,}?WÀˆØ>Ž?ï¿ÆÓIϾ?x§ÆÀ‡±È?LŒM>²;Ä?T<zœ`ÃÄ?|‹¦Àf?vF%ÄÌ(?ï€_€€Ž?yý­³Æ?]íG0Ig?GgwùJ©?Œ*wQ)a?y ®"7é?ïJ1íÁl¥?qT›å°"?`¢pDA?@y€:s&'?"¶Î¸ß3?q.Ϗ´?ﱶ×ÿ1?rláÅwVð?Y\KÌÜbÿ?SøB'列?€fÀ|ÿÿX?p`…Áík?ï?\ZZ$Ë?""Åûa´?Yx¾:ŠUß?d¦ÒP"?–|èËëWP?'»·á+Ÿ?ïøbIB·?"∔ÇIl?hCT	_Ù¾?V쫼µ?š¸‰4KÕú?ƒu0Ób`C?íäÙÿv~?Ãû–Ï?vº'ãºC?bD螮¼?®è ÖKR?u_e†»AGN4FGL J1717.5-3342?är‰lGH`@'ô}ë¾*À8:¯^&üÄÀ:[";"*Å@#ý:¨Èa@dc!7ˆ-?±LžŒˆ?Ã`à?›Ku@U£ãŸw)@4´g¦,?Ð87~òNg¿àÁQ'Ò­¿æl«ÅHg¿åðQ£"î¿ì›]"°§¿ã‹Ú"5¬ŠAGNbll3FGL J1717.8-3342TXS 1714-336?é'ÙÈ?ŸüTyÔØ?Å:IayÁ?Ÿ6¯]ˆî½?ÇÝ
Ni'á?À‰Û5›Bf?í oGq¿Ç?¹žë}'ü?s¢yuåoé?€ËÂHRìÄ?µÂ^,š¸Š?¸I¶û{Í0?àNèQÒI}?·{›7?·ç¡ãÍõ?¥cêñ\ƒ?ÙhFä©è?´®dKÔÌ?è{¼ø!?¨þlV:UY?‡ˆ+9Û¬?oˆT†?λ?̘‰hór?¨nˆ£º?áZa©É"?Æõ¥F~?±—Bëü¬¨?«
!9C?Øål	­A±?ÅâÎä Ò?é´ÓLKe¸?ǾpÇ®?ƒ­šjÂq?"nѼB2w?ÇñÙ)Z?Ç;Ïjré?àäžPÉ­D?¹ö€9÷­?¹£ã»Fñ?¦ˆ$‡`ì[?×Íʘêòþ?¹9¼™‹ÈD?ÞëÔAÊR?¶"x‡Èƒ3?¡ ݟq¹›?­§_ÙC#?Þð
†Ž?¶*p®‹:©MIXED4FGL J1717.6-5154?²Q†È¤À "ön†ÆÀ9r"áÉ´À;x"íˆ.7@šU'þ@%!4y?½nýùëi?ؼ‹ ¯ø×@¯œ…×E@ 	%m¢Æ?ïû—áÂA¿ÙßND0±y¿çœ/`•Áô¿èÎ,~
L¿ï\˜AÒ¿ïš@¨f¼AGNfsrq3FGL J1717.4-5157PMN J1717-5155?ë8t™7¨?¼éWV'ª?»&Ü7ÎÎZ?»K¼/à\;?©~ÀEÖ?žß‰pŠ4T?íw°JW‰v?³"AÀ|¢â?rb=ÞB "?'?Ñ3\Kw?³YÏ؄Œ?²òXuq?åôóµ~õ?³R«Œ?ÅË_*n#Û?®4=Ýü¸?Â`ÔЖÕ?ª"uÉüP?œyâ‰?‡«‹À…D7?Øñ@È
Ë?jI'ºg""?¢ÙåÞ'?"ümEËÈ?ê–Aì>I?»B–C"?¼5[ʉ¯?¸¢í<Ý?±?®1)«‹*?¢^pJ3ä?ëGõdgÖ?ÂÔ8;…½?‡Í‹á
¡Ž?›œ©÷é8Ç?ÁcRé9Ž?Á°‡X	½?äûB¢Öö?³¿ úÚ?È(VÇs,Ú?°—_Ïp?ÃꞫ™Ó?ªÕ°ÿš]?êÛJ ¸?¨™´à[š¼?¢þæÏ}7V?kŠCŽ•È?¿¨Bͯ÷?¦ÅÃ<vAGN4FGL J1718.0-3055¿ïíäŸ|\@7%€ÃÿÀ9<,†pÈÀ;Eˆ×ªva@–]Z#7@	•övê?º¿Œƒn_?µÎ–?`×Ë?û¼µ'•@ø§üaæ?ï}!"Î~~¿Ý]ÅB"пèw¦×o¾¿Ý*Ü·ü[0¿ç#ÑÌk¿çx×ì;AGNbcu3FGL J1718.1-3056PMN J1718-3056?ç+É©ÏE?ºº±	€dó?wCA¯Þ?j%é¼Ñ:ó?ÑK_¨Úí?º…•Qqã?ãÐüԟ?Âì\£Þ±?¡»€1.Dc?Ÿ)Û«ç?Ö&—âgò5?ÀϚ$·x?éÝx{3I{?ªD*ô—¹?'^"£d?‡XÊ䘰?Æ>K±›ª?©K[N(ƒ·?äç'r?¡ðE§óÝ/?¦Èà%«F?€"§‹ûnq?Ôó!vXˆ?¡ŽÔT?ÞUVãUi?Âñ¼aUì'?ç˜Ùiä?"x«ß؝Y?àp˜™ÊÜ?Âå
áã?ԓÊ3rý?Âj÷\dÒ4?­´Áoçd?²ø§V|«¦?ãÚåbK‹?Ããl\°Á?ൂ@6¦Û?µ·7+Ê?¤™R‡BqB?'E?¡ÁáU?ÜÑ.ŽçB?µˆÚzL‡?Õlâ]úÿ]?¨Oø¤U?·D6N#W&?–M£]#ô?âa'͝?©\Dõ3MIXED4FGL J1719.2+1745¿ÐH£>ÖKô@<†`ÔÀ8®j}L\À;®z¯É‡@B.'åue?ÿwÓv4:?¤ô^¿±Žá?¸??ŸÁëŒ@_e©Oð@"µçØí?ÐÞ;Ÿ"X¸¿Üÿ"Év7¿à!,jº¿àÑÍmÜ|¿âÎHÍÏ+L¿èÛÑLŽNAGNbll3FGL J1719.2+1744PKS 1717+177?ïòä#w÷?Gý|!vÊ?<CcÏ$?/]ho?S³qàV½2?CT»GJý?ïåm"4o?kö±\ó?>Žú°ê?LE+åK•î?fÀ‡¾)	?gJùí?ï¾Î-KÆ?yàëÌom?bëÑ«Ëù¨?q:zÂj?w#¯ ëí?r"®ä‰¡?ï÷»îƒ*í?6*£Sº/?ÿ¤¾Hë>üŸÁ0þÜ?OJŸ¼@‰?5g' ڟC?ïéêŒÑ4;?Uó˜HJÄb?="ГQòì?2XZèiJK?bbØý.¬Í?S¯\ÿ&g¦?ï«QCƒQH?†ë
n
¹?T—Y)½?È?c´5?¿•ý?'˜ÃÿË\?…/ï6"3®?ï¬Y1?¾Í&*3?l!± 2zP?x–2ÉæD?{ë#/î?v0§ŠÄyÍ?ïìT½z'?SÉË}þƸ?!—~.?±çÔæ?b'r%ÝÅN?SB¸XkçÞAGN4FGL J1719.3+1205¿å+ìï@9ØÈÿ¸²dÀ:Lí=…œÀ<4•äÙ3
@!; ¨×z?þ"ÑH\$?»1)ÑW÷¿™I#W›?àä†&ö@RgÎÆL*¿Ò亼)¿è	ØÆÖÇ¿ã9Pïܹ¿ÕõúX R†¿Ý±ª|ÀÅØ¿ÂlF9Ë'ÜAGNbcu3FGL J1719.3+120687GB 171701.0+121016?ïÐAF¤Ý£?cZ$)¦$Á?Ið¨Q
U?5‹ ;Zæ?t¿>ã=ò?aõ ËI"?ï¿´K-Œ?yä»Ôs‰‹?O]þÜVE?QæßaÀµu?|:9 ÚÙf?wfI´¡¬;?ïtx:¬×Â?~£D~ç<?aLGX
›?d"7°6?ŽžRjIå?yÛ>9×~5?îê©åþ2\?{ÈX)ÆE?bß?Ÿ¶ìÌ?D«nˆyh`? 'm¨áu?|d‹þ ?ï˜ÖÔ@<9?w=KÑ>ë[?ZM
­<?H)¦SÒ?†€©Øê;?u‡Q¶]¢?ïHîÐ`^?•Ëjù¨_÷?_ÁR£þÝ?j¬Í*H?•'+¢Ja?"XÄõå`G?îÊoŠZ?Cò'[?k$¾Û±?eD/']ƒ"?¡«×o8(?Œ<Ö5†h?ìg Ƨ¢N?šõ~xª+z?}ÿ™‰Æ–<?j&¦xò}?ºç2]}è?›K»6į"AGN4FGL J1720.0-5101?ë‰L
¹jßÀ‰êpKÂÀ:^Òn¦À;~1ôo@ڋIõ—q@À¹Ü/@_?ä/IŒ;?è?üÚ±'Þ@ g–@ý¦oëË@?ï8S~,UÉ¿ájzÈ:£¿éŽ¬ l¿î`ñ²_c¿Ûn€m¤?Vérí)ÛéAGNbcuPMN J1721-5055?ÚqIgì½?Х寚À?¢%Kvï?¢¾(S¸A?á¥7B"?ÐÀÄ_"¹§?ä+U«M?ɏJÞ0ß?ªþžÑ C?´<©ðÓ?ÔI)'kD>?Æ	ìêñÈQ?â¬6=:m?±rEìV&"?¼¹Qý›A?§›/¨TÁ?Óy?8Ô?±+²0Jh?ådZA-á~?±?+¸Ç[?µœñ¿Å#?¤z…|2(è?Ï d~t?¬·LœD?×E=?Ëh^–Áւ?µ‹Œ»ý¬?µPV|àç'?áÃEvùÿ?ÍXFRŸµ?ԓcd~YÍ?ÍWjBÄe?ħ¡jÚzœ?Å`² ½Ô{?àŒeó"¤Ò?Ìô­·M<?Ú>–Uc×?³M	ðn?ˆ8d0½H?¯ôý9ôdä?Ü}My–«?µââ€Ï?Ó#õœ¾€ó?¸¯Äˆ*'m?Á‡á5dÎ?½ ^*"ãˆ?âäG›S?Àekp‰MIXED4FGL J1720.2+3824?ïöù#Aùu@@̴ἩÀ:¨–ùݧÀ<pÍ_™Ä@bl¤CÔ@͘ÚVù?Äíañ34?µ>M˜-…?é·ýgŸKŠ@Ìٌù£¿âSQ¶«ù¿ÄGRºb¿ê"'úð̆¿éâi·S¾Ä¿Ò+A!]s¿ïûÜàSúAGNbcuSDSS J172010.33+382556.1?難êç·V?ŽRµ¦âÏ»?^åÖÔÿÐ?]wþ[;˜8?¹
}¨f'?Žüúñ0?ḯÃdX?rïB›@šÈ?K?#"¦à?S+S¶ '?u×9õ³™?nú‰_A'?îýLŠ®Uz?C°úv?V!;cTJ?'›Dº×ó?—«^¿e¥?…½9CÞö?ï¶tB"q‰?_†o¤âOÑ?`Lvï&?FƑrê­Ë?|»8[)\?[ÙEñnÊ;?ïSr/J%?
DÙp@§?q"iYaýj?r4_c€î?',ŸÂ¾Ü?Œ7×T1§å?ïwv8bêR?‰Þvw¾n?]}àO¾]¹?dêq:™?ŽrµØ~+¶?‡&à‹|"?î=ã?"OÈB¹?‹¼9ñW5?‡`#¨¼ý@?¥?Ö½c
Ç?·£û^-?ï!2ÃT[ª?~WókO?x)¢Y¾±?he&aÇ?•Ïb±Ù‰ý?z›Ì¦k¢AGN4FGL J1722.6+6104¿â­ÏÝ)N@Ap\‰mÒÀ:2ì|•|ÔÀ<WÄ/oYT@n
I¯÷@š%™í|?¼•p•x?¶7¸¨þfx?õPû«©@8"XŒÞö?·äùibð¿è™‡+¿é‹K¿ì&+¾ß¿è!p}–ƒ»¿ðAGNfsrq3FGL J1722.7+6104GB6 J1722+6105?ïø1½ÅÑd?Luøæ°ºí?<"ЭQ?I†"Š¤/?@ðÀFª|÷?5oXwޟÖ?ïÕL^cžÇ?rôXŠæ7?K'fóyý^?Uq2ÑÈ6ö?qôãíÔÈ?mñæ·WŽ=?ï õì´Q^?|Éq®K¶?a­Ù{µ•?g°Ëåž6?ƒWd[Ç?xٜþ ×d?ïàð¤Ýs?M6rºá·?S¥Û¼"Éc?9àÒeÈâ?e<mCMPL?H'9ø²ˆ?ïô½º"ÂÉ?V,I
"2t?G'ZL'¸?R!"Ðæ7±?ExRþͳ?DiÇò+ä?ïZE5?ˆY|
L"?XÂvxÕnO?de«©²-Ÿ?‰¡n×?…)\£ãØ?ïPôðNÔ?‡C:ñí?pãcßé?vëÿ'°?'ÃÈc¨é:?ƒ†¹o.U?ïŒQ_Ì¡â?rkñ¶«>?t:%ߛX!?aQg—çt?'Ε!YX?lÔ§	AGN4FGL J1722.7+1014?æ7žõ@8M¤-fkÀ8ù˜zµ¨ÄÀ;ãn)©G@Z×^K9å@qû9Ç¢?ªc,u)?ªÙ¿4¢Ž?þáDŽO¹@!O[?ʋîظh¿á!—à¿ä99±Êé¿âwÜ{~¿å¾´`šI˜¿âgƃ°AGNfsrq3FGL J1722.7+1014TXS 1720+102?ïöºJØÛ?AÍ°Ñh?)€-ݔãU?:\®?N¶É;+ÿÕ?@˜¡Üx#?ïãÊ'ò?iÙ!عˆV?>æ'?HàEëïå?hY5±«ÉÉ?ePu9'?ï¹é¶ðö?qù׏%?Z*JÖ6Þ±?c4–Üb-}?|ñx{XeC?m†û¾D!W?ïÞfU}®?P;÷EöG?L'!(&ä=?0
,ãšlÑ?jy!þz=b?L¯@ÍVSý?ïðþ:-"x?NœDŽÿ•ó?5u	ÑÁÒi?%^¤a±éL?X¦I?	_?Kô.f™™?ï©_Ë¡)?ƒí•ã`Eé?RptÜɸ§?`"é$Æ-?ƒZ/»ÍR±?î*ƛd?¥þE¯?~	˜éq!n?c7ôêpÓ?feL"'õœ?ˆ"ÙDߕî?z1æSôÛG?ï¨Íb¸ µ?l¥xϼl¶?c0´k•™í?Lì¿f-}A?z*;Þk?i/9†ºëãAGN4FGL J1723.6-7714?¨ü:‡6À5Ë6žË2À8J¾*ršQÀ;Ÿ0µªq@¼n<c@t@ylÓh?Ÿ¡"
R%?¹?æàIV`@4·õ¥3+@
5"Š¶Ó?·ßW=ÿj¿á&B‰èK®¿ãX—Ü*7â¿ä'ô¦/ª¿é±k«¦·¿â.•3ÙKAGNbcu3FGL J1723.7-7713PKS 1716-771?ïՔ¸oƒØ?i8ä÷à¨?Q´Ï›'S·?M>™aq$R?pÈoóëc(?eÄ.E=Í?ïãöo'?n®Ä]Al?:æq2Ði?IUb?h­,'4$/?jÇßï;§?ï—MõZÇ?ˆPÿ|‡ù?eu)Ë,?tÄòá¨à?"ÌÜð/™?…òz0r¹†?ïð?ëÓME?B)`oÑGG?1h ¤?Ñ½Ÿ¨'?[8Ý4'?@3öÑ6‡?ï™.Z"ú?|rõàÖ:Ó?`¹ß
<?[ñ½H}£Á?…†$E$ds?yp›7M?ïÀ¡üi?€ˆMG'´É?Gµ´_{îô?]™gø¹?|úxjî‹?u•D& Ö?ïX°"9?'ÞÌhH'?vÔ¨·7oô?€:÷4çŒ?Žq¿yÁѶ?—K?ïÙ<²7ö?`˜<ð÷?Dgˆ¥U?5?íÇ<kË?pÔµÍJÊ?]‡šÊŽ\ŽAGN4FGL J1724.1+3304?ïEÎñ½Æ@?»XK±À;$Ÿ¹šÀ<¿Áõv@ÄÑÞ¯xS@ȝ»gI»?Á××WjJ!¿µE@¦ä/ë?ï$8ž×ñï@½´«î±?èÚ>Oq¿î|b¡µÇοÇY¨‡s&¿Ó³ä¡Q¿á'óU͒¿Þj~yÊAGNfsrqB2 1722+33?î3']ÌJ?ŝ¥•®Ûÿ?TâCLH™?sù™•5Y?¬¼Q^Õ?Ŗ[n<?ïÏz¾&»?r h"y·²?H‰¾ ^!?Pa)5}ޔ?u1i;«/?oK–§"èT?ï1T˜ªþ"?‹:´ÚÕ?cç±ª?l"k/ā?—e/ítb?Š^&íMÍs?ï¸é$˜w?^"™t‰)?Yæ´×ƒ?@-Ðv°?}ÏË+ÐO?\±H)"ïÖ?îÀ#"4Ä?¯rÔÊ!k?eاQ¸6?uŽÏË3·i?¢­0ÿÞ9?®rö‰ãè?í@N"?‰2º¶v~t?WьƒhK4?b›ü¶¤‹H?ŒßS$NÅ´?†Ý+´,?îp¨ìjCb?—È"K·ìô?iÖç'Œ?lîq߬¨‰?§XĂ/Ø?–âø4y?ïž))ß?4ª¾áÑ?tÞþ¾çzÜ?fRC?U
Š?˜Ô|iit?gDAGN4FGL J1724.2+4005¿ßTãéh@@'dobÀ9biAâù_À<RS‰êÐ@fëÇc×@§Ös>»ý?°ô¤9/Ì?ÁÔÀa.™@döÄíÛ:@Ž¦‡é˜à?'M
`!)¿â~€Ǒ$¿æ@&`¼Ù:¿ç—áìèì`æʤԿïýø‰9™AGNfsrq3FGL J1723.9+4004S4 1722+40?ïß¾GŠ{?`¡8xÝ+~?X¥ñž?Õ?Q:€¯ì?c®R¦?WÉ"g˜Ép?ïßYUBü?sCˆÖ&âs?Aà!ûäóÆ?J½õ0
G?l.¢K4?q¢µÌÉ?ï°»
qaÜ?t´vÎLý?eÍÔìüL?ezFŽÍíB?}"Ñ)çÿ?mËLr‰W?ïõ–IziË?6!ú¦Çô$?0°¾Ÿ¦Ã?âb"oK?P§=Êz‡è?3Mœ¸A¥?ï½ó'M8Ý?p®Ý‰lª•?iå÷Do¬?`"¸+÷õÛ?t;0¡Ü?ik"Tº²?爵`…?ƒ&ìªïø?R¬y~Í?bê¤j­CØ?ƒûTÃ?0'æ=^u?ïnX¤B%P?ƒÕ¡¯€X?ts»7Eàä?t C·!Û@?Š/ù]r£–?~è`«b?ïãÎnãc?W&•ÆÉN"?FʺO+?5.Ë¥_ÚÑ?f¼ƒþ-?TY»NxPAGN4FGL J1724.2-6501?îÙW	Q7€À/Ç$ p¸ÐÀ:¹n$ É9À<DçԐ@8O§³
@ê/~r̦?ÅÕ^fWM?£GPCۄ?Ý܏¸oH?÷<í–ÆÖi?مâ,°b3¿ê~íEé]¿èS¤Wb½d¿âr‡ÂÀð¿ä÷ÞþþxA¿ï뒠+.,AGNrdgNGC 6328?ﻅ"0H??vdæÚ£"Ò??Ñam–y?4Q±UԖ?€"_ó‡®?uÁY© ¬?ïyö"Åš)?—Q2
?jþ|äo¿?p®£*?ŠÂ»ß'5ø?Š9&Ç|ò=?ï:"H¾W?',£ß7ƒ?p{ñMï¦Þ?mü|š´¼€?"€ÈÄ[?€}£Aלz?î[uðÙ,¾?€æÅ¥Õ/?ƒ¶2Ýôü?d"7Þö;w?¥[7j[†?}Ýø|un?ïHº
5%?\g¾àc?R›Àq¾îò?G$æÈ<Ô?•ÒL®þ\q?ŽÖ3ÜYn?î@׋Ú?®ÌÖ'¬{Ð?€'8Ç{ºñ?†Øýjvè?§ÙôZ]Ù?­L@ÑO•?îsrù?'ÁVqÝ°"?€d<DÈ¿ž?zuÖZçð{?¤¶	ЃþŒ?¼8"–Üm?ëQ¢'âã?œ'ê÷ÜÐ8?›¨¢ŽßN?"?<
(…?¾ˆÆÎ1?š6Îú'
AGN4FGL J1724.9+7654¿ÒãÀ™¸£J@?9¦ç_ö
À:¥ìeïH"À<^n£KÊ@¡@-lŸ»@¦;îך?Å0‹x™™Å?Š,†==ŀ?Â{R'L@	1‰èv¡r¿Ö5²ÿÇ ¿ç$w®G¿é¢
qÊÛ¿å`ø0'æ¿ãÔÄ}ròf¿ïÿïn¸D€AGNfsrqS5 1726+76?ïëvõā"?WÉz{Ôß+??î¹–'ã?4ú®vÆÒ?`‹I"Ÿnp?TÝQîÎZ?ïÙ§œo?‡?q¢á·*§?E4Vd–¯?P4Шp?p…¦é}xw?lB›S€¢&?ï£jL
V?yhE©{?XÕh@Ÿò?\¨6—Ї?" ¸m€r<?x.—4ó#?ïفf²?OIð×G?ID¾ì±@Ì?,|E3¨©›?pµ	r֝?M›§Êä‡*?ïØKÍw±V?oK9JŠ¤?M¨ ãôú?G:è–	p?p%'¤m?k¤Ea	y?ï™`ŒÞì?†ÊJ$?S
@9ò»?bÊX¢G?‡F{¶ðò?ƒð€™]?ïS	O4º?†9a7·Ù?dííòÌè?c¼Õ»`LG?"¸bõ}!?…-e+z
?ïWžL†Á?px[jŽ±
?eJ+kÂ\Ž?Qcžøãˆ?ŠWŽ&&Ž?o—³lRAGN4FGL J1725.0+1152¿í"­éª@8yLýÔ»À7éÇ88U²À;*µ[–ÿ‹@°\ô͜Ö?ü@—"ìck?ŸÃËØlNn?®}£;P[@Öâdä†'@
s—ý7N?暴f¶î>¿ÝЎÃ|Áò¿ÜWí'?2E¿×QDX­¿à"$݅Û¿ÝÃÎ ‰ãCAGNbll3FGL J1725.0+11521H 1720+117?ïßεìFÌ?gð¨dü¨?FÍf«Ä!›?C~ø[ã1Æ?j}ðbRi?e'8
ňÞ?ï[šE*p?åÔPfÚ1?vs¾£J?{¾¿cBȏ?Ž´ÔÑ?‰Ks¤pï?îéYå_Ò?™Ç/˜¸·Ü?{Ø)¡2ðæ?"#¹æ'ª?›çjRœ>–?—±y†¿ý?ëm=°R‡?›ÑN¹6òú?"5_¶³?rRyŠˆ—,?¿"
'g`?›lRT.Ø?ï¯F´;Ó¸?}ª©°iÊ?S½F>u(?N‹ò.¶—Æ?¶ª-þñ?{·"èÈ0|?î%K‹f?²ª%}Éø?DÔ/œ}?šƒ-8˸ ?§ËA1xö?¯ÂIˁòT?îLÙ–Ùm? XüÓG1º?Lð*kTµ?‡©+'¹?¦ß3;G¨?ž,âÍÖg?ç_Œyd^¾?°Kò2ª$Á?¡ÂóMúS?‡úB™3Á?ÎU3?°mÖ*jVAGN4FGL J1725.4+5254?ƛÿ~¿'k@A
ïܜM©À;°£µ|N/À<Ó¿jäz@ ¬Í÷ó—@"0Ÿ<¦?")JÒ¿¶9&ôŸ?õe=ð%—@ŒUðLƒ¼?åãÉjÉø¿ê¶u¨"ÉY¿æ­}±Ü†~¿ãÅ6jö ¿Ø6]_+´¿ÆŽån.\AGNbcuRX J1725.3+5255?益Ì¸?|;ÓÖWk?R[઒ù·?G)û˜nS~?ƒŽô¨â£?€¬eՙ
?ï^æI—ðï?Ð³Ô[Ëþ?rtíÜ÷›7?wë"n×®
?ö¸–zy?‰x¥ÓðŸ¾?ï;ÕðE?"óÓþ˜—~?`JxýHfà?L¿#öQ‰Y?–{òåqP©?"ØÏЈ?ïR´k¾%P?€ŽMÖº›Ï?`lV^Á4s?O`÷VNfœ?"›ç¿¦Ðb?€h2'{!œ?ï'­}žˆ¹?'reŠè?d^='Æ?Wž‡^~?˜~ˆ'Ì€(?C½Ð ?îÉì?%Q?¦"Nöá‡ë?|7õûEaX?Šk´ýúÌw?£|b~´Â¾?£Z…RQëâ?îf®ZQk?'Æ–Ÿ5²6?k¹¦ý?9?c¡ÌkBŒ?§ÙŽœÓoZ?'l+ÕÏ]~?ì֗CÉG?¢@ù_öâT?»p2‡Ü—?xØ«'c/?·ÕwÉ4?¢Ž'jL%ÓAGN4FGL J1725.5+5851?ì¦ir@@üšõºÀ9ó+w}À<'\ä¥6@O²×-Mì@g­Ãó	w?±ñOŽÀ?žmã;åŒ?ë?N_¤@-2¢""ø¿àžóu®¿ácAM¨)¿äļþ"°.¿Ý»¹^Û؃¿ç
ŸàÛwŠ¿áM20±ÏAGNbll3FGL J1725.3+58537C 1724+5854?ïùŒi8‰?7à"í_äÞ?(9]ep?¯BîµoZ?C¿÷z–T?4›é%…?ïãêâ¦A·?j…ѹ9	??s[šIèj?Iš—)¾?h&±¦Eñq?eýK¶‡õ?ïÊûlكP?cÝ™½Çœ?P$œí,P%?6©ÑæôÉ+?vy"bè×?b€"¼ í?ïó'8)V?8§«óÚ5b??@ÜF?#=S薗S?QÅW£Û?4(Ybý«¡?ïð'¤hç?qU›T½?="ãè}ó?Gp\i?XšZ²œ«?lj;+¨ç?ï®ç&?YÝ?'ºå"Òß?Nðìõì?[r4	xÍè?'W.HëfÎ?KjTy?炙Þñp#?qÖÚ!á?XŠ5Ât´?G€	œ[ð?'ÿÁ1|¬?o]è"Ü¡þ?ïÞÑÄy?X÷"*á à?UãO:Z"?Brë×°Ã(?fú¡båú-?S­ÀÆÅÓàAGN4FGL J1727.2+0644¿ÞàŠ†x¡õ@5ÇÛLÂPrÀ:†R{ÍÖ¸À;ݗkÖ@ޛÇÇ)u@—¬úŸmï?ßB"úùZõ?åðBrÁ>?ÿË.LC¥q@	$á‹Ë¥°?ï/›™N?¿Ýsdѐ׿ëmµz °¿ê3­Á錄ïÿý¥\Æ?Ü×æ¼5CAGNbcu3FGL J1727.4+0634NVSS J172720+064123?ïeäD|u‹?"C:ߜU?yI­ý5–¬?wp)T(s?‰ââŸÇÜ?‰«|Aa?q¡h?¤÷ŽïÖîã?'n˜/Úx?–ëò±k?š™Ç«"ˆ?™EhàD?íXSDº]ù?¡ˆnñFÌ?›cͳ;Q?"Á4UV¥|?¬ÈäÞ,Ü?šsaŽŸÇY?ílF__áè?'ñU©eû™?Š2f>)Y¶?r&'N–Ló?±W€=;Ŋ?'Ä®0¯";?îó'e'T¶?š¿ÀÌ?ƒßÞ®"ä?'á蛿ù}?—«#þ¹Ž??–õº/Oõ?ìCðùý²?¼'<ӁÕ?¨ÝîÐl?²¾–ŒËŠ??± ±ö8ª6?¯‡»À–Ö?ëÕ ¥*á?§N€Ð Ɍ?¦GbÊb€?›GðJ™µ?¶P×&û"ö?¢Æ./å·?èVº6‹q?¯P«@Åsæ?šì:
]"Â?'ºïeåb?ËGHž:¤?®vZ'àùAGN4FGL J1727.4+4530¿å±P"t:Ý@@¥‡+À8qq¡-ÒÀ;ÿ+Ü&Üä@Jž5àŒ@'eŸ—
? p·ß;¢?µq"Q³ÑÔ@?Ø2\@|Ë¢Ö.J¿È+ç—rx¿ãšG>'òŽ¿æýdQµ¿æ­ÞÎW¿ë#Ÿa¯g¿ïÿÍ'ý AGNfsrq3FGL J1727.1+4531S4 1726+45?ïÌÓ`m[¬?l'>–Ž+b?gf•{sß?^ùŒœþ¢a?kÆ
5m ?cˆ|'³×9?ïÂ_ï\wX?{=ñtï?QUí)0?XhfÈÄ(?zzÂêëÒ?yJÆÖFPÐ?ïr[ù·?ŒtGJxfr?l¯/Ø0ÀT?tò°/¶è'?ŒM°.}ä)?Šf°ŠG?ï÷Å4Ž8N?3\û{%¦S?8çt*ø ?$²D<¾ñ?Dwtµ
¨?+2ÑúãÃ?ïyWßó	?"ŽË…0X?mŽØ)à?dÝr®PŒ?ŠJ[ÿg¦?"\ÓÓlÈ,?ï^¹.	}­?'Yv«èX?`ŒI†‹8?k€3íô^ê?'Q#ŠÓì?'²äíu¦Û?ï›â
ª?—é¿x…µ¨?rAéãí¨u?yªløNP?˜|	Fíӗ?–dþX÷B5?ïëXÆ6?T5¦~§k?PÄB]Ê?è?E¢ÝeU1ü?Y%#ÛĐ?JòîZRAGN4FGL J1727.9-0654¿ÝÇTÚÅ*c@. ½ì_9KÀ:AíHmÀ;Œ¿®Xë@±F ù4_@Õ%t.?Ë*"<m2?ĈSvÀ5?ú§ÇúÕô"@V½sé[Ï?ïýª R¿æ‰ùž<°¿ã~ÊuÚw°¿å¢>ƒÉN¿ïõ}$îÌÒ¿ïë%@@AGNbcu3FGL J1727.6-0654PKS 1725-06?æu,^F¡?Ã,p<dE‹?‹±˜åúÞ?ˆ¾™S.Ãe?Ò8'Qd?Ã6b_,?ì|åT
ÌÀ?·ƒ¡µ.æì?¢¬*›Ù²?Fj{&š?²ÂÀtߢ?´º!Ù>7?æò¡F€%?°!¡Ãz6Õ?­ËÉ	ÒDd?ž>ñUl?̈¦,O?¬•ÛM\îÝ?åÆv
À›?£Ê#›­Éf?©âÔszÅ?ƒ—Ð%ý¬?Ñ7v…(¯ˆ?£À¼ó?áUñì?Ųu™ÆK?£¨?籚?œ–kõn?ÛzMúðÝ´?ÅL J@t?çR2'"u?Ʊ…˜´?¸. ù¼ó?¶qµ˜á_?Æ *[·ûs?Â`aXyWŸ?â˗©»Œ?³YÀâÀ?ºÊú Öµë?§±&+¢k?Õ!ª(vÛm?°ßD¨vbO?ÚµTžpv"?«{"㟺?µ¦½Ì,R"?˜®O~èO?ßàûîM{?­BË#üÊÇMIXED4FGL J1728.0+1216¿îÜ(̹@7ùSÞ¤e¥À9,ÂËÂÀ;Ì4–	Â!@¤é
ìî@qÈâ\?±\Á! ?·›‹¡´EA@³¼?¶Ï5@€'4Í<3¿à#Cf‡–¿Þ
D<œ¿æcˆ€l¡ê¿æk:ÁG¦¿êœ€iFëw¿×ú ø2¬AGNfsrq3FGL J1728.0+1217PKS 1725+123?ïëÞ,h
M?Wcì,D?Cá¼$^[6?8ƒCtŒO?^RÉ^àÖ?RäQKî\?ïÖ
À¥?uâKÕ狿?Mtþ'{É?Wv.l`;?qLYãá½P?rœÐÇ·pæ?ï}?«çy÷?ƒçVvf)?mÁNNJ›o?qWÅAË<?‰?ÁkW­_?€†NéÖ?ï¡Ê`òð3?b^zÄuE?cönÕoÒ?E"³Àfo?'ÌûW,?`=:gو?ïқ'@ÑE?pôôº£¾¯?V³¥9Xë?Q~Îì|Š~?qUsʌ?k~_S½	h?ïl(©†:†?¤vû:¨î?bù"@À?Æ?pƒÂê6DT?¸@™eQ?¤)?LBº?îóù'§?'±ÿœ ë/?~ÜÕ#úƒ?;¼wG½·?šI˜Â‡Ž?‰'W¹vð?î㴅á´n?"®Ô'Í?€²
&é?iz÷F5×ó?›0(ÁßÌ?g7kÙò?AGN4FGL J1728.3+5013¿»f[ã@@ÄÁæ¯ÍÀ8'û¡ÌnÀ;·–5df@ Ïÿ1N?ü%Ê_4Bþ?Ÿûß=#?ˆæ2	Μ?ê{`ž{V@Â
Җæ6¿äŒšþ§±¿à:þƒ©¿ßý‡[ח¿ÐþD4ã¿ßlL#Å&¿ÒèoÀ';¯AGNbll3FGL J1728.3+5013I Zw 187?îáPËۜZ?ā-UèX³?l'L†©šs?'(ÅrÅ­9? (~{ëd¼?–åbÖö?ïä†<ù
P?hyē͏±?:H^Xx‡?E…Lõ†U¼?h0¶þò Y?dÃ6+¬Q?ï‰)ù'ln?…dOKFï5?SQÈ9Ø?BiÕ-K?‹K`ÏÄ;?…H$nå´ý?ïîŽÈ§›‡?CÕ4èÛL$?!ƒñL.€W?
oÔâvJ?`XøΧa?Bá!&é3?ïÈ«½³I?­þè³ö µ?J[ÏQ˜Ž?€™«>)g?x^À* º?©îÀ¥g§0?ï²í´'?*pӛ¬?JEy^?Z9߄ëMË?Õ ­Cun?ú/¦Ê?ï,¬47%l?€Ý
H1?`IÕþÑ	#?fĆª%?˜a>²ôY?‹â«À?ïÛ,A;Æ?]Ç`qòÆ
?3<'oÚ²?%Âðh¹ˆ¤?q63MÌDô?\U{£®*AGN4FGL J1728.4+0427¿âI>'áy
@4w%_5½À9†…˜ZÕ9À;®MnGÜ8@Øõ¥@x<¢G¾?¸á(ypÚ3?ώLßV½&@Q\þØ<@Š³áŒ?å÷$+Ž¿ãs…ô¡'¿èc¾yå¿èA~O'7Ë¿ïéÈ@K·¿ï¸ 7­ì7AGNfsrq3FGL J1728.5+0428PKS 1725+044?ï²ÿöè ³?tAsüõ´ ?z$ÃR«k¥?p1æϦʛ?h¶'f)Þ(?^L	Âh?ïbYZ—[?'pwf‡×!?z$Mª<Zø?^Kë1?ŠW'¨#e¯?†yÙv-¢³?îœ$<º	j?™=l~Ãÿ?•cÝí?'PÏ,KÙ?—´ÄÆ­Ÿ?ŽÛ±UÈÀk?î")«°?L.±‹)G?¥h§¨þ?n›7]pf?¥ôÂãG–?{û…
+((?ïFW%3sÓ?OÆì×çÛ?Z»ˆ¥Ø?‡=¥W0÷?ø¢GL?{¤,ëÙH?îo{2ÙÐ?¥®Ux?€g4Ó½?—ä+êè·Q?¡/Î}:¹?›?!ÝL?í>ßõH?¢ã›/Î;?¤=ÚÆ©è?šÛ,H/?§Ô3jÝæÈ?™U@¬Ì?꟣£§¡?žeóL?¨­Dܨâã?Œb¼½Ôð?¾¬E´?šzMؾAGN4FGL J1728.5-7303?éÕ qMÀ4$ýó¶E¢À:Hä.bÀ<3+†–‡–@]îþOý@†Yùp™Æ?Ŧy{ìài?È5>eÁOì@Ü¢,æ@io‹þüJ?ïò';׿閗†™â•¿çÙ­…ߨr¿ìƒ[i³"¿ïͪB^Ia¿í³ð\ôÎAGNbcuPKS 1719-729?廙)sI?wcy{†Ô?bZ¦(M?UØQ¯"ñL?€ÈŒ%†°?töSƒ0³¾?ï*' 8\?"N³$+į?h½¹Hˆr?…Ãξ—êh?'ù]#œ'G?kµ(íê<?îÿÚ¥Ê̺?ˆßfÛÀÖU?w•OH"þ?sy¼o2˜ÿ?šd-ØԎ?…ˆ0Ñß$K?î'Ü* ?|<C(þä½?'ŽrI"?q½^@?›0µ†]rd?tV¶ö¥­?îþe….ÂO?–—CÈ`?y8ɀ€-¹?s ¾š¹ª?™åõ,·?"†ÏÓÂ~M?í«»"Uˆ?«bÝ"
%?˜›K+"±½?žXbE.-F?¨ö¢"›?£^ë®wS?í`P‰ý'³? ³Øæ×/?u¤JaGû?ˆV^MÁ""?°à
,é?›ïï\Hõ?ëÓïNét?—íòƒ·ýT?«@dWÅ5?åÕuÛj?³ÀS^.E?'uZ7=ŠÎAGN4FGL J1728.6-7448¿å
¯£ú¤)À4ó*®)s—À:ÄÎG÷–À<QiQ@Ã+Ìa˜@TÔ#&v?ʧ¹"ÓÝ?Û3ÿµ­K@LÛzåy@
¢¥Em(¿âîó2'#"¿Æþž–ƒ—¿åœ¼™xâj¿írJÀm˜à¿ïÿ—?LF*?à¯:ëŽYAGNbcuMRC 1722-748?ﳡ´‰ù­?z2)WÆ@?`\ò'¿'"?ZNj•q­?~¬—ßðj?v{Ñ9Eg?ïmkT{œ?'¹®OÇ?v>®1›Im?"oD3ž+'?‰…Ó¹ÜøB?ˆµNŠŠZ?î8D?¨•?™Ày‡t`Í?~û"¨œ€?…äÎÿµŠï?¤›ý L‡µ?•"qÛ¨?ïOÖ;Õª?t£í KùI?oulÔï¤÷?S@9æ—?''›Ó?r^M-ÔPY?ïcݞgoâ?èÓÿCÒ?lK'r´?kVß{ù:?õΨ¢c?Œ~68a x?îBD7a?ª,°û˜?Œ
iUþ?—F¬±?¡	Ad|Àì? 	:ž-õS?íe²Õ]rª?¡Ñ'ÀÿÔ?–qä0Ý?ð ;Ÿ=?®¢·4Ò?ž©ñàO?íu¬+äØ?—‹ºfv_5?ŠŠÏãhÖ¿?v,dM	°œ?± {ðm?•?تrýAGN4FGL J1730.6+0024?Ì®ƒ>¿@2§Å¬À9;z6'À;¹ö&bjX@|ó€À¯³@«NoÑI?±Í .ɗ
?Âòø-}½@ìÂ
V)Ø@Ž»NöY?ï`8_¿¿ÕmÐ}†h¿â}»'!­Ð¿ã3øŠÀ¸Â¿ås•¹:¿ìEUt¦›
AGNfsrq3FGL J1730.5+0023PKS 1728+004?ïç=Ώ"?`|\=®À?R,f"dR?ZÊ<èQWG?_Wü˜ýÊi?P@G@›Ê?ïãYIÙy?nÝ|'`¶í?C3ÞUÊbp?R¬à"D?gÙ¾tZÊñ?iÕXҁð?ï'ì4­Aþ?'fœž?lH:áCÔ?s–²˜!?"räD͎?}W‹¥5¿5?ï××û²›ý?TÏ·ÒÛÑ?@(•¦ƒoú?(èbŸý&µ?rïo® |?Szô¸°'~?ï×´­'?fmö'
G?Y›²¤ˆ°?UIeŽ¢8?lr
XþZ?`G4É=§¨?ï¤Çm{S?ˆ/îªo8?Zwúäho?l)iŠ¥p?ƒŠU­~Le?…WQ³lw¤?ïLªŽÅ'U?ŒlýöK²?vØ6rlò?|õ•KÒ¢?´ ‹DO?ˆlNR‹wŸ?ï'Ú/XT¢?tdÅ›ÙÇ?U·=Êã?B´V±ý0Ã?ˆæ@t?sž\>÷¹ïAGN4FGL J1730.6+3805?ïþ²Åå|ò@?ŠDØw$ûÀ;u¬Wâ?%À<Ìè^ùŠ›@!2ÂÄá
?ü `'çα?Ôy:éàÙÊ?Ó1¹KÈË?ü7«bï¹@´=«\9½?ڊ#¥ ¶Y¿•sÂ^M­¿Åûá¸AO¿ÚÒ²˝"¿ÞødÓiI¿ïÿîͨ"ßAGNbcuNVSS J173044+380452?ïo+9ÇÞ? é0ð2¹ƒ?c´‡œB©?l_O©0‰?HÑ=ћ?Ÿœ!øÁ?卑Ñç‹?€{HüP†?Z†Fâܾe?b}ÿžÖüC?'Â¦Åßm?zӜ""í?îknè¸]!?ž¡×5?Ž2ª¿_:ž?O{ìŸ÷?¡¼fÁ2ÃT?™Œÿª1Ò?ï'·î³?}.Æká?tzÒHR¥L?Wo´VÕíç?™\Thß
?|//Ü|CN?ïeó–mÉ?•·Ó%t´?k«S'è'3?k}Âø'?Ñn)û½U?"±Ë¼÷1?ï=Çè¦5ù?'E"×	‰?hƦ8זŽ?p1ê×Ñm?•..%R+
?Ä1yñZ?îifS¤ ?žåˆâ:'æ?Œhøθo?Žw$
vAB?¨_+e‡¹à?›l) ¡^?í?ó˜h—?—Ö²"ç?ƒ	'mð…?s0ɜ0@?³ŽÂ´nì?˜TïáóÒ*AGN4FGL J1730.8+3715?ãrO™¬u%@?WðgȗÀ:NqªgG7À<ˆ}@@úÈi»°p?þ>ΌÀmC?Á×¢é¤sè?Ç=×&ñ@R4ebZh@)ߥ¥^?îìPá
¿æèm<C}-¿ÕÞ½ÛB[o¿àÞYçþ¿âš8%
|¿ïùK ½OVAGNbll3FGL J1730.6+3711GB6 J1730+3714?ïäÆÿ?[<
ý\?S¢)·fº›?H°C»ð6?agëÝgÄ?RÝí0òr˜?ïÇàUÆd?vw~^Ñ+â?U褄ZHp?]ÀÄUÚÒõ?v•Î:5ˆ?pŸÓnv[?ï¦ð ¢³…?u< ÜP«?`þiTy?^Ú±%ú(?'#XKzå•?rúÏòú'Š?ï::ª\Ä?m78ˆØ
S?|w†!'O?SÆÆ?kX?'•LÑì{§?ký_=/'?ïËxžn·æ?h,¥•x'?f¿Ô&z_?Xãa¹Vkþ?mǍ-\§ô?_r¶ƒBÀÉ?ï^ö¢€•^?ŽDî»lÏ¢?i'űÑz?r…\
°Œa?ðê¹FÞ?ˆ¨£ãÁÓ?ï^Ò=‹Ä?ƒ=F¹ ?q¤«v]ûÄ?so͒u?yîÏÉ/?~~ãÚ3Sq?íõEž½e?ˆ"‰CÈó?j¼†XŸ?q(¬,q?¨vž¶Ç¤Z?†çàêà	öAGN4FGL J1731.6-3002?èyÈøú·?ÿ'¶@™MCÀ8èšÆÀCRÀ:ßPÃfò}@÷–ýˆ•@HËwb?·Õ÷ÃÆhÛ?ÆCž:h0Á@
uÐfµ@¿@1{ys‹¿ïþ}êªr?ïÿùJYQ¿Ü¶ûª¿ãA¾qg¿æsßVø¿ç£5ÄÝëAGNbll3FGL J1731.8-3001NVSS J173146-300309?äŸû§©?Äfî¼ûb?¬u«:ÇJ?¢]ùDôÕ?Ó?Ùü­‡…?Üá»)È?ã"\ò'?Ï)ZnÐ1?ž•Yßh‡ˆ?©^nˆ/?×ヨ@¦c?Îێ±‰%?ãΨçë6D?´ø*¾Åx?¶9¤9ÑJ?£ÅÅÁq£&?ÒÔE!GMq?²þm6€Î?áümGðÉE?¬²tÉåï?¨l¢
Þc?'XdÇ1Ë?Øù'.™¤	?«ÅY6¹5Ò?áh°‰†b@?Ĭ³XBÈc?µŸ»
œU?ª¼ïÂ<'?×ìvþ0"j?Ü=ðÙ½?ÙHßо&Ÿ?ËwP¤™c?±ËÊàÊW?»õÂFXv[?á"»X[6?ËàoÐâ?ßÔå\]…?¶@°NäC?¼ÚæQ>r=?§îŸrs%?ØôaSHì?µ€9OÓÕ?ÖNò^?±×‡Ô´È€?³ŠŸ\7t?™Þ0à83?âg¡S;*<?³á$ÊDPMIXED4FGL J1731.9-2719¿£7p'`֊@GëäÀ™À9-	¼AdNÀ:ßÀú)&@š¤Êû'@ØDŽŽoš?ÀÙÈ]ÒC.?¬øæÂR†œ?ñtŒINþk@{9ºHf?ïÿMB}þÞ¿ä/½BNF¿åA·ZtÀœ¿è,›Ÿ-WQ¿ç?B5.µö¿ÏDxjtèàAGNbcuNVSS J173149-271928?ÈdzÄÓj\?¹Ê$`c?€yï"QÍÿ?y4¦+tŒ=?é¤ù"û9?¹¤fˆ "?ácçÀH?ďÔO^HF?¢ØÄ:¢«K?žU#M+É?ÚÝu}ì¦?Ãí—q!<?Ø#~ËÉ'ã?µ(w¬—Ÿ°?©Ý¯sû™L?š-ƒóti?âPe¢épê?µ·!!µ?×Ë \¬S[?¥0´¼€f|?¢"6û€?z·êŠÎ?âø†ž$'?¤Öàˆ&»½?ú>]fk"?µu¤Æ7?†›|ð+ü§?mžC@I?ê·u¯?µëGj°t"?ÐA»tz¦?ÂB¦@¤"{?«¼Ö?Õ<?°Ìšc¶6G?æ#Uqª4?ÃVr÷ÞT?ʂ2Ê­Â?°a»v8?¨ê£0Œ·?–ÐÈÄzNî?çÐÉOR4?±HÉg¦÷?™áR?ŸVäWß?©i˜Vâû?e×»·Rq?éÃ"÷ѳ<?¡P˜wDTûMIXED4FGL J1733.0-1305?ë{åäc–@%;À n À7†€Ǒ$À;
ì-4ì@õ ÿÿÕ@ُ¨?›dN^1ä?¿~™
,¹G@"? §?@žáW¿Á¥ˆço»¿àãÀ~౿äásLþ¶T¿ä.×N0¼¿ê:ó¼$ÞÝ¿ë.HG—nFAGNFSRQ3FGL J1733.0-1305PKS 1730-13?ï}.pù	?fõ¸À?ol'ÕÊܹ?n¼§'9Òq?ˆ½"µ.>?Š£—¦#?ïJçüj?£k"œ±[j?hÂbƒ²?s'YÑþÿ?"Š½°: ?¢¯Ö95•^?î´Î?àã?›Ç{¶!3?'³_Xúë?"õþB'V?–Éæâyf±?"pj^358?ï€ "À´?vy¼§<z?k´·‰o!?]õÖ³¹×?‰
­7ná?q®Ùk?î"?·ÈP3?¢î'qŸ-?ˆ›ºF''?"þÓ'—Ò? ¥õEøï? 8öš¶?î)Bà`Žœ?¶hw¶»?ÌC­,]&?"ßÒ1<mW?¨øÁ
Ðó?´Ê"òuQ?îzùYXòò?žÜÜÁ4ÞÇ?"Ï=ÃċA?"œÙc4âô?›Ñ—õ¬•?•‰Bݕßà?î£ԃŸ?'>øPm²‰?ƒ;SÀã?uy¯~;Nö? ÿ~ÒxER?Ž»Îµ ¯dAGN4FGL J1733.4-3943¿æ§ZìÀí·ä{õÀ9cßÏpÀ;oÅYa›@­T9éç@–-¹v®³?¹œRÜpÙ²?£dûØ(¯?êúâm©Q@p
xä¿å îؐO?ãæóŸI†Ý¿èä^ÿ"Ë)¿Úâ@|q뀿æ¤0ÌP¦¿×@êÁTs AGNbcu3FGL J1733.5-39412MASS J17332704-3942172?êªoMÑÖ2?³Ñ~.ÏÂ?z­wý$žê?¨'¦R³®?Āטˆ€?°í»O úv?ëšjg' ?¶r(çTã?_Ìo">d4?k<k›M†˜?ÁV½'h5Û?µ±fm[óÓ?ëØDãðæï?¦8¦Jé™?Œâöeê˜ú?†þE»'ï?½¡z§n?¤p	_F®Ý?ì´*;è¹g?)Sïo?†°î†@D?e£^"'À?·ˆO…½?ŠÅ̯Cðˆ?åœó«³Íw?ÀHóÈÓݧ?~ºÂ ÜS‡?"ªr(M?ÔK->Œ$?ÀVÙ¼°†?ä¤ua ?ÅQ|áõJg?mÐôûó1?yäX¹i?Ö|!+ÒIl?Å6Úì[o?än+øèoÒ?·
ïþ°=®? Õ›ð^R?–l¨ÝŸÒ?Õô‹(?µly ¶á?èa\¦ÊÅ?£|¥Ô º?œúÜ汋?–t´§xë?ÊÛ1È¿{?¡àj'AGN4FGL J1733.4+5428?ëÐZ—Á@@vÿCAž0À:"Ž÷À<m‰5žG~@MTùLˆ@å!ÂÈg?ËE'Á(?Õù"›…¬þ@ I@¼?øÜWYX6?ï,B³Ù¶À¿àáô±î$5¿ìÚ _†xU¿é¨¶7_޿á"Z¿ï÷ö'õ;AGNbll3FGL J1731.9+5428SDSS J173340.31+542636.9?îõOÇW[Ë?›-d77]?€.ôgÎùÖ?|Ûÿâ"?™>ŒÝ½m±?—Õ2ѕ]?ç:c™™2?ÅçópòÓ¿?ÈÕ`	ò?ÂÈq—œ?´'Äx¼ëˆ?§¨^ƒn	?ëžáÁóÍ9?¦3'0Ã؍?§³å¡å*'?—ù ]Û	?·.ÿ!"Âs?¡Is¶aú'?è£ðíéR?¤š1‡³?Çâ'õ3ì?£ñ_g#
?©…hz¶×!?ƒeñ"^ô'?íæœ+Å*Â?¦gÏæâ´?"ìÚ¦'ŸÓ?–ýÉ×Àiê?§Ïî´5ú?Ÿ¸@½y6'?ޖf<0C?ÌoA8t?Ø©ÿÿeb?ÍLi:+J?"›3ˆÔ·?³ñ4°í»]?éLԙõ´ø?¬³õ¦ºÞF?³AsLǼ"? õµC+>k?Á+óóF"?¦AL‰Bä?ß<nÂø¯÷?³\£Ê?Ùßþ_c_B?´ÕÜXšë?»ŽKvÃ?š¢w‰…l"AGN4FGL J1733.6-6054¿ÉʞƒRJÀ-{¿PãGcÀ:÷8±!vÀ<0Ò­·]Ð@\U"°K@°h:{üÑ?¸ÐW›ÈH¿}Ëg<½/'?Âø4È4@+Y%¯g?B`Í ¿Û:"dKY¿äêkäT¨Ï¿âôšÜ¸o¿åLã=Qš'¿à•ªA°sAGNbcu3FGL J1733.8-6056PMN J1733-6055?ïõ9\0ò*?Bpÿûžmî?)8~3P&A?»ZE6?Rf8LÎÌ?At»Ôöa?ïéŸy`Ò?iŸ"C5Ü?.ØWmÒ?<=|Dž?dsº«?g{Èè?ï²03¤r;?t
VA5˜~?X k	U?«?`«n¢Ü΢?€oåº0GX?rR˖¤A?ïÉëÿÿ?TÍÒR!Å?L¨ìÆå¦n?*ÑuT	—Ê?wÜìG@ý:?SÓ~Éß߆?ïíQ¦?P0õ_'¶?9¯ 5‹ó?&‹)ܘû?_'vµqò?M@xéâu?ï´Ü'~?ŒÛÄ|ë9Õ?B~
¨ð$?SŽ
­©
?¡…ùÉ?‹Ø³ìÉDí?ï?µ;zn?[üO¦AW?`žk¯^N€?\3X"<ñf?ŒwÍàÖÂ?|´?³WY{?ïb`ža¥?s#nÕ2e?ey—Oû0‡?J'a'ôé;?'¹M>!N?qñ¢"‰AGN4FGL J1734.0+0805?ïý-&Ì
@4Ü^³¾#À:{÷öFCÀ;ïÁ¸œ" @*¢Ø\¢î@'¤ŠŽd?ЕGûAT?ÝûÈ£GmR@·üƏ›ê@ç‰>W©Š?ï³Ä¾
'¿áî)°•	¿è
¼`îØ:¿ë\4-n¿ïÑÙ|¸[¿íññIƒ×AGNbcuNVSS J173400+080628?î9Rz²^ô?´É ÞI†c?Mmß"5?'Ågڃ?¤D!cš1¯?³ìGš×ò?ꁡ,'af?¿¿qžÂ'%?ºµ{]ª'?¸¸'ô‡þq?±cA ý=½?¯ 9A¦NÅ?êò‡Üس‹?©¯Ç‹è¿?²RÚÍø½?¢<ç[×1Ï?¶çþwm?¢É›Ažâ­?ç·&MØ·"?¡…ÒÝõùs?Àìñ°[ýØ?—÷'rNi?À6uA% ?›h°*`Ä?ì¹][û©Y?´WÃus:?©™	ZT†Ö?§˜¬<g?ªÑ 脘"?­nLŸüñ>?ãrÔ²¹"?Êêþ†XIB?ÑÉ7Û¨?ɡ˙hhÂ?À,m¢«ø'?±r¾½?ç×è¶Q$$?°.6òu÷Ö?¹Kêm<[Š?¤ƒ;gÂÙo?ÃúgðT;l?©'öM«'Æ?Ø·Äh‹jé?ªTñ™¢ˆ?ÔÇW·åë?±)!ë8þ?ҀãßQÎn?¯ÖPÍ*žBAGN4FGL J1734.3+3858?Ö¨횀R@?%á;ÛÀ8B9ҍ×À;¦ôlNô@`A–{@ÓÛÝr?òq»ÈÝC?µØçžp*@S,ü¸Lã@âà‹OÕ¿ÎAØi¿àW-^T¿äi\ð›Þî¿åÜ Ýp3¿ç½ŠÒS¿è§"ïQ0AGNfsrq3FGL J1734.3+3858B2 1732+38A?ïèoa.;?Z§ýâzÓ?CdTb)^?6rÆ«$x\?b™‰_Ùê ?Wµ×A·±»?ïӆº;G ?sYZû?K«0›ÈÉ#?VדÑãÊÜ?rÇ<ÊH©‹?pe>jî9E?ïÅýž·÷º?y| n«Ës?YíD§Ôä¬?i…6eU?v…ßb¦?u(ÇõL½?ïøýp"ÎÀ?3%`]±>?#æúøT	?ìÕ¿f£?GÊ
@V?1æÚ±Åõ?ïÐGʳ±¸?sOüžõR?@U‹êt5÷?7ᰆS»?uÑi+(E?rôà­Kr…?¦!	?•žÞ(ʘ?[HûýSÃ?lwµü?‰ÒzJnÅ"?•ÜË çg?ï¢6Ÿ1?…%çv´¥?]àWšxî%?jó5öÀ¾Ý?ƒ¶MMËmÝ?ƒkr—ßž£?ïîivL¸?Q!Ô9ËLH?8.$Ñðf?(Ÿâeo‹%?]"s¹ˆfß?Oíñ­Ëƒ°AGN4FGL J1735.4-1118?Ðàø0†c@&p9ïôÀ:J­£;ÚÀ;Úv¾£>^@ µ[ÀE*@Cò%Kéã?ÂÍ1÷sê^?°
$àÎÑ#?ìÜ蹒]?ýiù¿Ê?âå=¿ë]ãà刅?³¹" k³¿à!ÑÁ©-5¿ä¾µÅ$b¿Ü|ö`D
vAGNbcu3FGL J1735.4-1118PMN J1735-1117?í$.ìZ9e?«'®Ý­Ø†?ptõÙ¿?_KHæ<LD?µ×H.u'Û?«>ó4.t¡?é7("ˆë÷?Á.†Õ`ˆñ?'Å¢¾W?ÏÆ&jwî?Èê«$[?Àw"hQo?í}qDç?¡#Õ¤æ"?‡ç|"§U?"~ øþA?´rœƒóƒà?žºZÕ¿?è¯4aÓÒ?šmÐó5ì?˜'ÿ%ú
?xN6Ë?mL?Ê>¯J'bè?™Ã1 <4?ë#H¤´Ï?´ˆ<tÀë?'L¹[Œá?s|áNö?ÂN`¼`÷?´=;¿ô¢)?áÒ*¢@U?̳ÆO²è? Q_R­?¤"ÀRH?ÚK€	?̏G"³¸?ê4HÀýÐj?¬Y*Q!?–·6n™>??‹«œë!b?ÄWö-©R?«
·Þí?àÊ/s¶5?§$‡Hß?¥‡jܱ‹?pfF:^ç?Ûº³¼ýÄ3?§;Ý6;ÝAGN4FGL J1735.8-5932?íLRÁv¸À,™¾ó'ªÀ:'çIOÕ*À<8pÇé8=@x/fŸò#@®œ£9UŒ?¿ZÝààô¿¢Ó›À\ÉQ?çGžÑÿ@a±"«É?ïòŒÝt¿éå»±–¿ê©bdy&¿Ò(>"$˜¿åuöâJ"¿Ý‡±d¼m.AGNbcuWISEA J173553.24-593204.6?íµis?}î<gÉÂ?Uù#"µÌ?IĚËËT?†˜à2ƀ÷?|4gb"2?ï¤fØbh?†¶QIïnU?W?cr/Ò?[2²¿ŽUƒ?"¹Þ9é?…p¡‰9?ï:Yÿ6?ˆ½^÷…~?m8ñnL!?e°êð)˜?™1´›<M?†ž½.™ý_?ï	¤ô^?u«Öð(§Ø?r›!7iïú?TÝØhÛ?š$´ì慡?s˜Ø'Ìu?ï}Ë¾–?'1:ãëG?ož¨Ö??cžÅš­?˜œw%˜™S?¶^ìâ{g?ïc^Û=å?'+"3ñ?eê+&OB.?r{þ‰Îl?›ÖN¾š~?œð;ðó¨?îtÖö¿?™''Êûr?zûÙc‹Ñ?rújÀlZ?«9Dˆ.Ýð?—Lj"êÄ?ìán¼:J?"¼?;E2?WŠç‹P<?{À–ÌHb+?´Þ§co ?"
»"#×AGN4FGL J1736.0+2033?ïÙÂ¥Æ<@9kÿCAžÀ:yÇQcÀ<4¹º¡Q@`Ý•.?ûåå½^šÀ?»%33^&?Âڅ4-@	qá߃ˆ¶@L¯d‡/¿ÞTÕDj"?ïùînD˜¿Ñ0oço¿ÕÊÛ[	T¿áþàzÿzŸ¿ç#pvóÒAGNbll3FGL J1736.0+2033NVSS J173605+203301?ïúÁ¶²óÍ?2júpCo?."'ˆž¦	?"—X;Õß?:¨õŸ4?*º¶é¥A?ïà¤q¨¨š?n%ƒ~ñhá?CašiöÂ?NϹöӗ??jƒN.Ü>^?h=0E˜¿˜?ïºæñı~?rg(·©?\ěÕýÛµ?b¾…ªƒ?{[`KC?p!­1£|w?ï±QÌn6?`´h ¦÷?ZCš]0¬?=Qȗ{?€cGÅ]å?]36~cR¡?ïö¾â¹'?Cún·ä¶?CJæXMj?<C"œ^±?A¹'{`'¸?3ý˜
©¿?ïªâd†	?ƒÄm5k$o?Uè°YØ?c"îLÃå?'ÁqNŸ¾Ø?[Ó«…J?l•ï/?¸ø§—™D?k¤Çúoè.?s*}×B?…örÕ¸îC?w¡o=÷?ï]™Å}<?wþTÂUJ?hgêâ0H?Sß*Š$¬?'?ÊC{X?v,>~–5AGN4FGL J1736.6+0628?ֵՙúÈ@3Ž7y…À9¢¼ƒ©mÀ;ÉÞuk¼ç@ÇÌIo4Á@ñ·?œÎ?¹gj3%?¢ähÂ-®Ü?áïk'–Fÿ@­éa'ý¿Ýê¬[¾Ñ¿å=yþHÅ¿êr(a&W¿âՌY?6w¿çiš-=Oí¿å‰á`ÈWAGNfsrq3FGL J1736.4+0634MG1 J173624+0632?ﯱGzç?z¼š©ÿ¸E?d6¤Æ?ZÑڐH?~Oc©id?w=AÉâÙG?ï°_0Ma?ƒqu[Dg?`Dƒ	+Å"?gž©zï~¸?َË6)?~ì°j0?íþ.«AÀ?™FëÀ»™	?":å¿È?Àfá+@°?¦'
'ÈG—?'ìEGŽ³,?ïžHˆ‹?vò²lÕ½v?|¼¸ªne?\Ï4"‡æ?˜ŒGÀk¼þ?s"€"\?ï/¡C–?'¡O4?
[µr½?}ÀUAdG?'†±BTN¼?‰Ñý¿¦?ï*/76^?—IóEâ€?s^t߸Ó?? ä˜ò²ì?•å<ã¾´d?'"ÍGZ?ëk'?š?«ƒßå?©-‹Fò7?žïs¨´¸±?»ßð¯š?¢§%«,¶d?í5ùwòø?""ÌO‹?—Õß¿?€4tz:?°r¾oØ?'G»K2<ðAGN4FGL J1736.9-3357¿ï¯šP½¿ñ];_QŸ/À9"#æÀ:cçl‹C–@'.TQ;@̧…ëfì?ÒyÜ>YØ?НkJѵj@i"a9×?ùîþ"n¿Ê±,Þ/u¹?çepûì¿à¡ÙÙû‰y¿ç.Â5D0¿ëcoÁXûD¿ïÞÜÏyOwAGNbcuTXS 1733-339?–©#!´?"wÓY€e?™>ï"Ÿ?®½K
e0k?ïx•µ?±"P%?´3ĜŠaY?´¾é¹†bÊ?³þîDpç?¬®¶«0?êùĎÝx?·£ Ɠ§?¿§Þ@g¤)?¦í­CÏËu?º©Ïdà2
?£ˆå…?t?èµÊKW9?­ž6f`x?§n¼M$?…÷1èZ=?´(*ÄäEñ?'‹ÍºCÄa?ì
»Yîð?–0ò+Ð?'ÑÙÑíóä?—/Em‡^?¢pYŽ¤?¡Ããcúì¿?îä]®m!}?«}°A¶5?¡ç$Ú?¥_&" á?µO}ø›‹ ?³ÈËîñù?ì7ógã‹?µów]¦ñ"?´JȽÀâ«?œf¾
"©?ºB$ÎÓ?£Á.·b'I?ê6FH?©¢NÅ?·†ï'Ö~?v_Hz"?³f'²fói?šÕæ×Y?íOËžé?›êžFÄ°OTHER4FGL J1738.0+8717?éÇ"A¯‰@;ô`RP/À:·9©MÀ<¯b³S@cÓù¼Äí@\Óû•74?À›íܼÙæ?¢ðæ t®l?âÍ*àÔ@´@Y‡2ŽÈ…¿î®kón!?ïý­_Ÿ!ï¿ç]à…ç5.¿ÜlOIoI¿äs¦¹Ù«¿â4¥>ŠFAGNbcu3FGL J1739.0+87166C B175708+871924?ì'q?ÄwO?Қš²À©u?ïCŽ­?¤?}2t‹?¹úÇðêÜ?ы	Ë}8Ý?ïì?U¢Á-?eénqäP?4¦Xb‰÷õ?B'Š1ñ?a+ßAò{L?aÎl×f%E?y˯'?†¯,ýäK?Oê¸M]7?8&µºˆÍa?†ßfìîâ>?†©Ÿäøþ?ïþm®%º?ëÒ
ù>ü½ªEw×>ç³ÐfÃ?%l<‹R"?_°ññB?îä¹×ÁaN?Äte
Nk?IæLI
Ý?x²1øîçE?¡LÊ™›?Ãõ2O;/4?ï»Ò‹ÐG?ŠW^ãD›V?Hgö|î‰?X…–\¦?£JCWZ?‰ŽÈôê¼ç?ïOdC÷P¯?ZªPc)?Y1¥d_k?^ZûIÈ ?"€]/{¥?Žãm€¿‹¤?ïü'$ø?.06VhŒ?;°ïõ?´ÚŸ;ñ?:'K?,~ÎÅBmAGN4FGL J1738.0+0236¿¢o˜‹žü|@1€*ýڋÒÀ:n@÷À;ÙYæ%cg@´Þ'›¦@ÚÁLf
 ?ÍùdÅÒ\¯?¾$jÃmR"?åü§…ëg@#+©&?éVˁ¿ØÀPýôb¿ì¥Ž¿öЁ¿íÒÅ4R$?Ð웟-WQ¿¢HtñoÄAGNbcuPKS 1735+026?íY"À?À Ó×zr.?ˆ³;½VžY?"öˆCA.…?°~ÊqŽô¶?¾k†BÇV?,˜­?®âŽwªñ?…iU¹€?WÈx[.Å? ÝRâî$Ë?ª‰q¦‡ÿî?ê¼DÁrs?¨™ZÞ· ?¤i–×ÔZ
?˜íhMÇ30?¿éˆGF?¤fN%˜d?ï«	ûκ?"g "¬òF?RlÊøo—?Guº!eŠ?žCÒ
ûæÔ?ƒècó
F?ìqùëF"?·FŽv'1	?¡QA¶å¢?¦Ñ+Îg?³ìˆ8&Š?±WfPï?í;ºY"ÖG?·4Ëd/?'©‰AUâj? üP€È}¸?±wÊäã(?²‰Q1Ú}?ç
'³?¯µt¸"?³0ºfZâ?¢¼#…‹Ý©?Ê?ñøbC?«Ù¿^Ü «?ì3»«‰¨'?¥ø£®/"¹?qñÜ¡?p€+­,œ?½C
£"f¡?¥[uS‹¸AGN4FGL J1738.2+4000¿êµUg:¡¼@>z'ÓºþÀ;ƒšSÓ½À<7‹öBçÜ@QÎCÅQ®@©ÚßµÝ?Œ)™pÙ¿µH@Ô±s?ò¿zÊÒ!@¦%‹ªÃŽ?ïÌi?‰­¾¿êúcÿÿå¿áŽá¿Î¼¿êqH'Š¿¦I`àÚ9·¿ïþâ=ø3-AGNbcuNVSS J173807+400312?ï¸uKAÙ?­í3ϯ?X`×RÈá?\ºÎuS÷?}ä¾þ§i'?©E‰yk?ïŠò÷ÆN?Ž7sx+?kaÏsÿø?|plH$É?†jÎ|¤q?ƒÍw=3r4?ï*±['?9çðN8?a}y¼¨<?i½˜Î?˜z%fëI?ŒvïÔuÁ?ïˆNH•ù…?r*¿"=A?Aº$'æƈ?7lÝýGÊ?ŒÐ˛/¬ý?qÆêV\?ïT»d€ÄG?›Õ®¤–î\?kEÚ{FR?ia{–áp?'ê¶ÓÍX?šº¾*¾1¹?ﻣ•¬?›úX˜9Ì?mP|P§È?|á⦅gÂ?™þ|Tˆ"?—0:ÿ\ z?îh¤=Ù̲?˜-ÓÝ>2`?pÁ2ïÿGl?r¨aNt»<?§]•Æñ?—DŹí|?íó/ ˜Àš?—UŠf™ê?c»åS?]ˆ«a;³?¯œL)çÿ?–³^GÑ(fAGN4FGL J1738.3+3228?í%êÙ¹Uˆ@<´›ùÆ*À;8Áo¡x‹À<}uôxãA@қ&·yÔ@Ÿ¾ÿ"°?Áø¹ò8¿»ˆÖ}АQ?øÅ̒ë)¯@ì|a$ˆ ¿êÓB1Ó¸¿ä̹ìö8¿étyN w¿Í{«ÝhüC¿ïÿÿ&¦³?ïÿûÞ]BüAGNfsrqMG2 J173841+3224?ïã‹Ø2S?"'#÷¥V?Wþ"¢'Hh?rîBò"±®?`tݏ¢%Ø?váŸÂz|?ïÐØÜ¿Lö?uh3ï;z?MÁ{:è~¬?Wgc!q™'?sÛb;/h:?pÒÍF3ñ?ïO1úV¦]?Œæ"¼•?pSŠAf›?x}{"W,?'Þ!Ž.?‹N*EÓè®?ïßÞÝpˆÿ?X‰¸ò@¡ö?B'Ýz"a8?3i3¿	Éj?k€kÏÚf?U÷>È3(?ïÆևÐ]??'oaÆߋ?ik-׃'?qHÕ,?o¾KQ¥u®?xWd,²¶?ï"Ài<.¯?Ž–Pü×2€?_)ƒËÀÌþ?pò½Põ½?Šêµ94ƒ?Š>œ:6F^?î宧ë
w?'GÆõ¸¿?vm¡am¼õ?{ôqŸ´®?®Â¬ª›ß?'0ÜԝIÔ?ïxŠx5é?€–Ê\Z?f•œ)®à?aO)ÜÇ?Œt¸6íõ?|¬fÒÏAGN4FGL J1738.8+3822?çÌÇޝÒ@>ȸkùÀ;îQ{‡À<ö¦€1ê@!ØÚøºº?üóìFØ
?ÔrIÞñ<™?°å#/Úä?Ù[^€=ýç?ô'=ìs±?îÝ\á0¿ïE¸põ5¢?Ö ÎAAð¿é{S]u&¿œÊîÙŌD¿Ç-q}EÐðAGNbcuNVSS J173842+382104?î"{â	Ü?¸"H¹·µ?ƒ­™_p×?´½—ÏLÖ^?¢ùŒÙ£½?­s½ëG1?îîU˜/X«?¢ùcHq?MK¬ã­?†ÉNNRÚ?šaú
P4F?ŸÈ/ÈßF?îƒË¾Ì3?–>Xî=;É?z Í)?€§]­RY¤?¤¡~s0?"9^Á7Š‰?îG>ól?'¿…-Õ9ÿ?eKޟ"T?[@SØ\?ª:Z–dàô?'¤hê$%?íæÏIv8
?³ÀBi ÇO?UgÊD'fg?bB€ýoBµ?°sæBg;?³°TÜé4?íK-?´Œ*‡rb?‹½@)ö$ˆ?š°¨Ñ3O?°o ×
‰?²7Ýde(z?í?q¯ê? P¤^áu?ƒ'ÚG_'?…îX'b?³ŸÉÆÎ?žá8ýhF?éï^;?±CRX³—?u{Ð&¼¶ä?tþ]ê÷?ǖ©H͵?±[¸}('}AGN4FGL J1738.8-3418¿îZlDn;i¿ùצ•*ŸÀ9O¡(TÀ:zòl™†N@ã""i·T@`ô¼ÕÞÄ?ÑÚ£Š´$?ѵ<O|@>EedÞ§@Õm¸?L¿æ"PA`ó`?ï%…€]˜¿é#Ê?SÒæ¿çb_I¿î'þ¢‡ÔË?©wìÎQ‡AGNbcuNVSS J173913-341749?Ç¢bålD¼?·éÞ¾Wb>?ÈÀûÍCö?ÂA
ìíÿw?ãç(ScÝÔ?Ĩ߅"²ˆ?¾n\-l8§?¹–g0ãF?·Y¶NIþÀ?°¿¹Õ–xg?éFý°D€ã?¼9	zÁÖé?΢ˆ;ßeg?¯+ôWXÁ?Ì~
v¢?«˜`g¶Î?ãt>nƒHþ?²ƒ«p±˜ê?º¸³©ÿÝ	?•\=ë|?¸…óU&ìâ?˜‰×ÞÜk?é˜+ñës?ŸMRDûš†?ÀÒÁ²¬)?´ujN1y?¼1HYW"?¹"	xÑW^?èE&ˆ*?Á59)¹¯0?¥¼ŸAÊå?¤Ö¸øžP§?ºô#úlSw?¸³œ¸=µ?ëE±ŒC^"?¹…mÚÒ]«?À…™;è?¥e*äöˆ_?Å^`ªÝL?¯`ÃõnÉ»?æ‡!ïï³?²Ñ•Ý˜9?5Î ½mg?ô{ˆ{ªì?»yÔú ì?¦eUÐY-Ë?ë§ï¨w?¦1ÌP²cOTHER4FGL J1739.5+4955?²Üæ/w+@?·¸€®À92`8NûçÀ<CÄzî´@!;`©8@)æ~Nº?§ûîxn%Í?µ¸¡ÄË@
_`ûÃZ]@ã¤bËQM?ú+ª©¿á^Z(j'U¿ä¬…>õ!¿çêÿè­ÿ¿å•‡9᣿åE~Y¢2ÅAGNfsrq3FGL J1739.4+4955S4 1738+49?ïï]ØÌú?sß9tâs\?EûŠ-RiÓ?sà!"ßI8?VGüæìmÝ?B¬OmÊb?ïãÇV&Žp?j
R¼L	?ANX¡®pS?K˜õoaI?gåΒ—k?dþáëï‡?ï­º°7S?x'-€ :?d±Ò~?Ð?p
[~Ûû?~ɾ'.æ§?q•'8+
?ïô==…F?7x[«ö ?7Ño`R
@?!&»Ú*?Q'*tœ®Ó?3nªZ€?ïè™"º]?W]#«£W?2¥B-ωY?%ié¼ëX?eŽ¾I?V0™Lƒ"?ï°þ ·ùŠ?³¨¾–?Pëƒ.貜?]EAOð÷?¢çjl¹F?€.Q'âÿá?ïq³UFGQ?ïy@!ôî?q.jՎ£?rŠEáZ&S?Šûâ}ÒØn?}0ªkÈ«Î?ïáۑ®
6?Vú«á?MHœ,?;whzCA?f½'ú1q?Smüc¼ˆŸAGN4FGL J1740.0+4737?×íÈ^ÂÇÕ@?_Ãb(À:< Ÿ²¸OÀ<aë­b¤@¾éõ§Œv@$§š
\à?¼åúÆ/O?±."AS?õÔpšœÎØ@©Ì?ïÿÍ_ï©Ç¿æX}o—h¿ã1Ÿ_VQÆ¿Ùº-Ç©­¿ãQ@¾Œ¿æä&ó|AGNfsrq3FGL J1740.3+4736S4 1738+47?í©°ú?Ñ2/íÙaÜ?†Ý}a91Î?¡.;xÁ?´ïÍ¿ÚÚ?Î\9"Äé?ïÙ6Kä8?qÜØíDL?Hhj¯A½¸?RÊBeã?pWå¤rG?lñÿœ'Ã?ï\;:
?ŒÀѨw?U¹a´ì?`a;måã?"&ðΗyÅ?Œ7Úµþ?ï«PfÛèZ?[^q«æ±?hRÍQ1îá?B¨Ø)í¯?~.eÖä÷¾?XT*8ª?…9«?Á—I"ƒ?vrÓò±éí?',I{Œx?¤%Í3Ãߐ?¿3kBß½?îúkŽ?…ÑSUx¾"?X¥i‡B—?cT'ÆG?‡J×/Jr?'ÍþH@p¾?ï°îk?"̈È-?\œhÓiy4?[:>ø‰?›SCXv7
?"ˆƹ7o?ï'!ûÓK?y1¦àcá\?€±–åY‹?aë4ív©=?•uMUi?v‰¥¶€€©AGN4FGL J1740.5+5211¿àÁŸ2=r…@?ÂU:Ä÷ìÀ8'Û¼SØÅÀ<#ÞËÒÒ@Eãdú@œ¦Êı?[œ"?¡ñ=;í
?ü.x?'æ@¹'ÇÅüϿϵšðg¿ãõ"!	ºê¿ç?']<9¿æm7:ÿ°¿åWZà f¨¿ê¡7¦®AGNfsrq3FGL J1740.3+52114C +51.37?ïøËWÏK?;þ¢"h)Ù?&˜Dëq¿·?Ä_Æԋ?G,~\Ø?:çÙD^¼"?ïà«äaä?ţұ,?;ËgWЁh?F§ã<}½?kÚ¯>æ?r3)'°I?ï–cúÙÙ?…Ÿ¡sí2?V+6ŽŠ?g
o§Ú?‡¡žÖoe?"oåäsy?ïþ›(ºß:?%&‡¤Š?oþ|A0">õV¡A¤ô? qsCÖé?Çoã¨æ?ïòñ2ÌtÒ?OêÕÈw?/Ôýš+§Q?"ª¡¶m€?V"û3è¼Ï?Nµ"Đâ?亮ðN1?uQ}Û?P˜‰SÇAŽ?^ïeé<éÆ?"+á¯u?lQ'9›?ï2ʦ	?'²Ï°îW?^3½ûƒXŒ?`¹o>#–¦?—ÃoaÿÒÈ?'yÜ_e6?ïüdƒÑõð?3]!­ž? C"ï[Ñ?*EÄû§Ï?4º»U7‰?0†ˆJ£>AGN4FGL J1740.6+5346?îÙdý"@?Úuy(àÊÀ:WÑù\xÀ<zp§@Xâ»Ìtb@ÀàpÀ?»Æ.£ ?½…®À>•@ÀÄù™´r@oo.ah¿áDãß»¿æ\ÄÞÁ¿âVÂïÔ8Ò¿àîÚÞÞGI¿â	w­¶‡¿êÕC^#¡ÆAGNbll3FGL J1740.4+534787GB 173932.3+534742?ïús€Â?2>=Ã÷0²?'ØvæF?*]Q?@=Te[g?-1—[Ly?ïâi×+˜?m*5òÎé°??Àº¥ÄÔh?I†(5«P"?iö~¸žíÃ?h]Ô!EÆ?ï΍†ˆ<F?^TœN|¨.?NJvùyt?9["(~ë?tïíÈù¹)?\@Ùæ›?ïÔZ
£½Æ?TšèÇ|È?WI3ä×°)?7ïo¾9é?p¬ M‰?RQ́Wð?ïö³'V¨{?@Ðåeäc?5¨ŽƒL¯?%dYõ€|h?J_ªz"?;©	ÝõBs?ï¦RÞ5?"Wä]¯(?Tê#°@r‰?`û¹¡"?ƒÎ;pBl?QE×ÍtN?ﯖ½é|}?m«í7ƒ?V"ûӊ?CY^![?Vo!oÂ(?jwBœ|¶×?ï{|p
y?rÞ.š'WË?pÞÔsv¥'?W*7^T#?ˆ±yÆPÂ÷?q‡Û§>F"AGN4FGL J1741.1+7226¿íýO&"@?
¹pޏÀ;	³Ýè~À<ÂDK‰kN@:äƒøž@êp?ň.!Ña?¢¬Okx?Ü[Á|Œ˜?ùšw_²íþ?ìµæSҐ¿Ü¼ã`7"V¿æÃr ÜY¿äAß¾–ÿ¿áP2芘u¿ïÿX¥³ƒPAGNbllGB6 J1741+7224?ïDšt¿?‡Xœþ®?Y™N}ãñÝ?R]ý@šëL?‰{¯›0?†7K#ª?ïI#S°ðè?Š2bÊ?tmÅ·ûöƒ?q×N-0Ï?'À$2ùa?Šìb*CU?ï4Ñ{æ³Ü?'<Y5"?uYQqŒD?pð˗ú?"| —7/?~ìRÒ†`?ïöÕVUš?vF©Œ°š?…•"žü(1?hw
\šÄÂ?"6bþØÀ?pþ•^óí?îí;KýÑÊ?"GñÁ§>?jÚI%M˜j?`"|Ô¢f??žýM^‡¾´?"ì–jï?î*‡|zhÁ?¥µ¨®_yb?‡KþÊ;?ÊšˆûéO?§u6@Œk? Í‡Ü½7?îvÐÈÉ¡¹?'5©˜è?…Ñ, "P?€–ŽwÌ?£¨Mñ¸Z?*·'µÁ?í%q‰ã¡®?'~Îúêæj?žÊßæÉ?‡—`[ßÌ?®CwkIä ?¦Äüÿ™AGN4FGL J1741.2+5739¿Ø÷"ÁME@?븝jßÀ;ø¢t4À<­2.@ö睸0@eÄ÷1$?Á"ÑöØ9¿¨Í¼ì"ù?è›NÇ@
JML¹ìö¿Ø…o«‰†&¿è"Lá<P¿èbs'ƒ¨l¿à"NÿA"¿à*6¡Ó¿â÷,ò§QéAGNbllNVSS J174111+573812?ïúì[ø:?36DpQ'?'N•'	…?Ê•G`d?<õÕÄã?0™µÏϓ£?ïáCéÜœ?h‹‹Ôz7?;&øz?D±ÑuǦ?kWR1Þõ?dô·&dD+?ïÅHúÎE{?b(ÿß9?N⡇½?5øSK°¬é?y.rOñä?a]Æ?ï薻݀?FÔ\]y%$?4-]ɾ|?Ø»çy?d㘖9gÖ?FR¡=êJ?ïö™ßÝ?Eõ¬ÒcW‰?6K		ªv?'‹‡^'›?L'l,8Õµ?B¦æ¼ãÇó?ï¤ê]V?À¡@è¨?KÄ濽þ"?Vfš¨µ-Û?…	0	Åí?€Z_¥??ï•Ë8™Q?qüˆé~wj?W'úä™9{?D¬˜cz?‡šò¥ŠŸ?pòGÔ2?ï«ÇMÔ@¬?iü¢ò˜—F?RélI»?Ag"~Á}²?'¼g…–?hýç+²³4AGN4FGL J1741.5-3119?鏿åw'\¿à¾+IÀ9CUÚýçøÀ:Äz³ûD¯@È©¿±V@t6¸ù±1?ËϦ›à›·?àÜ{@" @¤˜"¡¸?ü(3/­AÂ?è<ÉIŠ¿è°«#.Ù¿ÐÄ?Êñ*z¿ásÇ­©¿ìzׁ܎Œ¿îpÍÝîÞAGNbcuNVSS J174126-312329?`M
àYÎ?z×Æ_
—?²K¡l‹i?ªiŽޙ?ízW«´?«¼z%RMi?·dú¸dØ>?¶âˊÚx?À3#K'-?´¯†·[ú¼?éà €m?»'®4u?¸ŠÎ¶§¸?¡|­,vë?ÊW"ú#?®œ¼촓?æXßÛzî?°jƘ¤Rå?¬=D␶û?!œ¡µ?À‹üìùÞ?¡JÁ€yž?ê,vÖv?¥¸¸K9ç?ƒÊD"—?vžª5Ú>?±xÓ¢6ß?ªÿu<sø?큽+2øj?¬ar»Ó8?ž­áòp?žd®-äå?À׆³§¦'?·He˜ë	?êÙJEbN™?·x޿笺?°€½4~aÛ?˜»ãùíŸß?É+.æâ›?°Úêqœ?祟r÷n?±ô,q©ä¶?'!ðMÿN?zæÚæw?ÂÂùܜÆ?©›U`£''?êìÿ¿Kô?«}ûªòÀOTHER4FGL J1741.8-2537¿ç;£u¡¨î@¢å€!ùOÀ8Ôê~ŽÀ:æ[{PÙ6@ &½´«î±@'ÞkZÂ?µqÞ>º$ÿ?Ûä'Z?ÜW!O Ñ@tKøÑãb?íø©)Y•ž?ëù>Dß-"¿ä΢o>¿ä8kì¸$Ÿ¿à½!Þ÷ò•¿äˆ×~×AGNbcu3FGL J1741.9-2539NVSS J174154-253743?ڏ€÷d¸?ùvìùñ|?‡U(_÷_¾?zò¢^	+À?âZêãí?ÃÞ3vðŒ?æ,}RwWa?ÃÑMiY#Ì?ŽBãÑâe"?¹ZÍe?Ò´î<fÁ3?ÃkûC
?ßó9¹ñ9$?µAíŠWhd?«Èk'jé<?š|6ŠÀ2Â?ܓ¸ÓŠoõ?´z•ZæÊ?âø6'¦Ið?ª¶µƒ5þ4?£",Ÿ;?ƒ?ºÉßA?ם2W|ø?©‰Âg]Ö?ÒTàZPáø?¾‹v"=Žù?—±ØžŸåN?'{î-²¥5?æ
Çú?¿'±'è-.?ÜR'Z¹gž?ɗÿtŽƒ?Ÿ³é î÷?°â€'Êc	?àÙkŠú?É¥Ýg"|?Ñý`Rûûd?³‹OtŸsª?­e $¿{?'ñÜ<0§?å0i"¨ñ¦?³äµx²à?Ö¬YŽ«mÆ?°P™Û¿Ì?±yXÕ:Æ?—†½°
…{?âz¨5ÏÖÔ?°\¿ÚD0fMIXED4FGL J1741.9+2555?ïí²Ž:É]@9ý•1ã¨À;,PFipÝÀ<­^éšbí@½!ØAõï?ï0]€c½•?ø£Ðä¿?é¾ý×0ÓÝ?ût8Ùeb@-bŽÀx¿ê×ëC°Xù?ïÉxQ{¿å4µê28¿¡ý Ãô$ï¿ïÿú Âî'?ïÃk$;H«AGNbcuNVSS J174147+255443?îä¦E­ø?¬šï…äyõ?Žw	•¸¶?©Ìs8@j'?"/²…ö?–Æš³¾ìŒ?ïY<w³'?¥szöì0?€i–žöÑ\?š÷À¸¹¼Ç?‰GK@Ž!?'vs…ÐèO?êzþ`Ï6?¬ö'W°ßê?¬Ã˜cÂ$Ü?žQãiʳ"?½Æ@Åܲb?¨Ìj#иÁ?ï;b€—ƒÚ?ÇyîÜÖ«?[
݇çI?kçñŒcìà?–âÒ›o`?ãܚ‹k?îrïƒ(?®9A¿?—Që˜'8?ªÙáH´î—?˜Š¦+Ðá?™oÌ÷ü?îÀVFތ?¾#¶'LdÌ?›‰Að€Õ)?·#wª¥h?¡ßY¢uű?¥{8"@ûM?éZ]5)q?¯®?uº+?©š<sý‰?œŽ>Ë"±?Ä/ü84Ø?¬·tl€µ1?îÔã®T€z?©å†3䝟?YÎevü߃?Žöš²U?¡ãQëÒmî?©i¤'øÃÿAGN4FGL J1742.4-1518?Òèô
Œ
H@פ?åÉÀ9Àºª‹YeÀ;_Œ™¦@*ò03¤r@1ú´f¤?Ðç=¼h?݆T"A'@~€8Ÿ"@¥uT ?ïÿÉ仿⸗ÁREG¿æ×í\M¿íø < ¿à— /µÐ1¿îôú¬)AGNbcuPMN J1742-1517?â!r¹•–?Å
n}È>?"غ§íU•?"gÁMD?ÛVMj'?ÄÃÆ^‰?âá¾ÃÂ?Ãð¾'²:i?±i_ÃÈM?©º|™k?ׁäŸZ…?Á!'±T¤?älPÍ;ÌN?±tàzDÌ?µ±'ÒaI?£y67I˜O?ѺúšîáÓ?®W%ԏ‹?â_hÓ©	ú?¦@ÉV1?±t\hù£?'0‹é Î(?ÖÿÑB8šâ?¤±"}cê?Ôƃ~òpÃ?ÃhÇöó?•5ò#u/j?'fÁN@46?äó¯4$d?ñ€BRw?Ñ2™eZ4?ÃUmIo?Á®]¯Ù?½fyº3˒?âû+ö0¦ï?Ä|8?Œ‡ã?ÛåÏûÜI?²‰Ï,ež?Â&\¶~?­ÓÀ!'ÌÑ?ÛâL»Åh?²Þ" `ˆ+?ÑøX;€^µ?©?"3ݦZ?»éî"?£K§4d›?ã¡ñ%‹n¢?­;®*MIXED4FGL J1742.5+5944?ìFj­m@?Ⱦ
í(À:(1ø .À<˜Â^§U@';‡j—ù@RI^ãL?¶WfwÆ?›šà|¾'Õ?å‰Eû7@·º×Véq?îú¨Ü,¼¿åÒÑß^¿äø!å-¿ßÈh"M×ú¿äpƒڐۿäÍÝ·×AGNbll3FGL J1742.2+5947RGB J1742+597?ïæ퍕2	?T4"'f¡?G´;"¯w?6$R¶Ù_ö?c%p®½þ?PÎ{W÷ÿ$?ïڧͨ®¤?r/m$tj<?HôDº?RÌÑsµbX?oSõz\éÃ?m3Ô]3?ï¬(T)o\?o·ò8®Õ?Yy;FÒHI?[I•¤ZPx?ÆÚàEÄ?k3å¸l<?ï¼RÃ585?Yn.•D@?k£ÞõÎã¥?Is­ÐR?t®Ü¾Ì?R$€{…n?ïÑâɖêñ?c÷K]ñØ?UPKyÕsÚ?D¯h§´£?qºˆ;H6˜?`¿àbþ=b?ï'4$—0€?‡ÈT9Š‡¥?[×"‰íR?f
ò€EI³?ˆ8%­?":èÓ u'?ïh¥'°¨:?|…×m)A?c•>ˆTa|?Uø¨u·?x¥ñ%M–?y›¶®Ã?ïFYw"_º?v'Ý7Õ¹˜?'õsän*?fÏL]Ò?‹t./{3K?pÙM6³&#AGN4FGL J1743.9-1824¿êäò»ý@5JœÀ:%N1¼:®À;欇²çH@íwÜ°oŸ@Ýœ®÷Ð?Ð3rôb³?îhOt²Y"@èK èBt?÷1=ª…z(?î»ïÐð¿ç±aË×Ú¿ÔÂ܉r¡¿ëDjÞEE/¿ïÿßéà
¿êÖj€˜AAGNbcuPMN J1743-1828?¡âCÓ$»Ý?œ•Lð-+?Ø
XЎ?Êɛªjø?âÛ/aJ%q?'‰ï¾¥~?¥¬8³žÕ"?²Ø6qÝç?åF>S?ʳÍl¯Ö?Ó2v]2Õ?Ɲ´†YöÁ?Çqì6I"?§ÄQùÓÞ<?Þö?õRA?³7؋&L?ÕPˆ¥øÄð?±'\q?—;äÈò?zUHr9Í9?ézËÕ£W€?¨uMŽBa?Ç#)+X¯€?§€é1‹?'Pž<¼Tø?ˆc{£°?Ú @¿ã°?Èß÷tÉ´?âríð0?ÈÜIHµþ?"øUm™Z?§"è§[¿'?åiPW£l?Ìú‡;©?ÓíÙúT;ä?ËM §CÀ?¼1'QÚF?£y*­5T?ḽè¶Q?¶Öò҆OY?Շ·Ê1<
?´W|õÃÃ?p…w€A'G?]$ân9æv?ê"lõ²ÛE?­~¨K"ý?Å. lå?­-¯Lʎ"MIXED4FGL J1743.9+3747?î$5úÈD@<è˜_ö"À;g5¼zo2À<»-0º²ï@g³îY?ÿuÖ[æ?çéR©ðÿ²?Ø*HþÌy@?ógÄՇ†r@œ*M[}¿ïñ4 ›–t?ïýìo¡Î¿ß¸7^»ø¿àͶ!Ãg¿ïIűO˜Å?ˆ`NQû(AGNfsrqB3 1742+378?ïjà°Ñ»ì?‰ž
Hš?vâÆX?pÝ݉y?‰Öpƃàß?"ËŒÿÙô»?ïŒӤ#Ù?}æµàXç?TúIøf—…?eRpŠ¡«?wøš†Ùï?uZ'ãÄ?î+° ¤ÙF?š'ïj×Ei?ŽjÁ®¥^8?‡nÐìa՗?¥ªEŒœÉ?—cA¤Ø?†?ï£-ú¹*?h

¼ØkB?aÈ	Íòõ?T†×$š&?'·Z§?dàF¸'U?ïš.?'°'\þ—?ƒaؤ$ħ?|£ÏQ.?\?•ËÓ}–á?¨ö!è…?ïM½j%°
?•Ä@@ŸÈ×?mƒÞGѬW?"Þs!?'—ÖñŸÝ.?zMD£À?íž? ïðàŸ´Þ?–ûÑ¿r=­?#6A?±hÕVò?œÐ§DI}o?ï>ËH×ùë?‡éxÀ€?aj¶pW?jüO›Í?•ù@"xދ?‡iÊAGN4FGL J1744.0+1935?ïºß'³@7SÒǸÖÀ9rƒ\@sÀ<ÀÑìÇ>@¼ß7Þh¬?þ"à¿ÈØL?±'×
hcÂ?¢ûW¾q¯	?óÄÞ ²'/@‰Î³£?ïÿÕØå	¿ÂMæ<à[¿áìÙ|Þwð¿Õ³~G-»û¿â›õ>…÷¦¿×»s^"0AGNbll3FGL J1743.9+1934S3 1741+19?ï´¢FfkÅ?uKSô…?I—ÿ^ج©??ÈzY é?=îd*ƒ®?t£¹Rþr?ï¾ë\Q\?}$Ýzn?[¹ºe/ôS?c–{¨%!D?z›¬Ü¨ö?vN"þó?î癒kZ ?'½=ø2Ô?qd¨êÎú?vwe"ªc?ž³ÍB*¬X?¦HÞÓûä?îÃh´c8M?y¬FՖ'?ˆÄ	jóúõ?e`oùW…?›0ä·?Àâ?sùmߕs
?ï^uÿê/?†¤çFê½?]*Iìéeõ?Q÷‰ÁaÃ?'^›c?·È?…ŸÕwÒ[?ïKæ¨›f?"XÃu"?oòIjÎq:?xXNñ¸¾?'"áі¶?Ž8Æ­µ?íßvèv?œm5"逯?~e†3䝟?|³Žá%;?®;îåHî?šêpšª–?í&
Ǧ•?'š†,)4?Hy·7?^0u0^8?¯›^Š!?Œ}Íaý^AGN4FGL J1744.2-0353¿í5¡ä…"ï@*B®Ñ9CÀ9Í·'Ò$ûÀ;…}Ý{pº@ÕpK¯@meie?Öø]i?³ás¢äñÝ?î=Å}£ô@+NVÀ¿ÕpÔ^;Ÿ"¿ã
8bGõ¿è4Ž}å¿ä˜òü¿èÙïÊþ–¿ÂÒ°X¢AGNfsrq3FGL J1744.3-0353PKS 1741-03?îƧÌ.¹ž?U.Xå?SfD‹©?Ký/¹mA?¢üð	 C?œÏØ¡ÀzF?ïQïС²\?•Ñ'}Üõp?jqF!ÞV?q>hœÌÈ?'sÝ%;Ê?"w"Sbh?í¿ÜýÀ?Ÿxà‡+èB?†£æ÷wÁ?ƒ²µJ€Pû?®YD½9Õæ?›ÄNS>#N?î-ª~?†.i˜÷'†?p ;ì›5?Od݇A*?¬iüšcÒ?…]›_Ä+?춞o
Ì>?³õH£	?j5wéÃ?dñy…ôb?¹y`ÆT½»?²¸u]íI"?îò`°f?±F#Øè³	?}¦æ"-Rù?‰#Pc±Ž?«LW»J;?°.@Uì¬Í?ê#Ý	…æ?®ü
Ûü?œ ¡Ð¾¬ ?"G•úŽ?ÃßØQTV?«Ü
}=Š¨?êrð™µ?¤2*yÅ ®?‰û}LLƒ?o5̈́>@?Ä¥ˆ‡šàä?£¶eÊb£ßAGN4FGL J1744.4+1851?åm¿²CE@6ø/@_k À;\ŒñšÀ<™ªæÈ÷U@!v<_+߂?ü²7Pþ?ÏyïÓ»©?ªl…©?܌xžÍ5'@"`PÍ¢á?ïée߭п형";"+¿Ø¥þ—J4¿¸þ2ËYZ9¿çàm"R¿»ÉÐn
AGNbll1RXS J174420.1+185215?ïË:ڂ©#?qv=Ñ>Ü?3Ýø7Sä?#ß'‹1?y$³ICè?qAÁ'›Fm?ï'ó¤kÉl?†âík?ù?`¬Êc'ûæ?eµž×Üù?‡WäG±¨+?ƒ=|I"þ?ïK–Æ¢Þ‰?ƒ!˜Ðt¸Á?XfíÒ~?Bt£Á»?•¸Oó?ƒ,ÅíGß?ï7î¨iÁ?w5åÃ}h˜?]£}Qq-?DÓ͵¥?—K7øÄ?vCzœ?W™"?}ØÈd¥tƒ?AîJ_¬ø?2'ÃM
e?ˆ@E÷Ü?}|Ëï‹u`?ïlCu?˜'_…Ž?fæ-'?r¼ž´ê
©?›5¥@¿¤?–Wƒë«ï?î®'Ãhu	?Ž>ŒO%¤w?`ýi(â!?Rɘ|C‹†?¤
­6¶HÈ?±0|;`?íƒ.®Ç±¸?"ç}‰¨†?qӁ‹ŸŸ²?c¤¨þÕË1?²ÉRpš"Â?"Ã˅õ®áAGN4FGL J1744.6-5713¿äsÿðÕYÀ,\8Ÿƒ¾fÀ:
ٖߪöÀ<L|f'ëØ@ DÁ^.´s?þњw+?¼¯éè ?±tÏ	èâ?õ­`öºÜà@xM"µm?ïÿþÞ÷¿æ´ÇóI8X¿áX(`s¤¿ÕÙjj%š¿ßWÛßm׿ää2pLAGNbllPMN J1744-5715?ïñ"RÞ?V	cNÙ?üŠ$Û? *WNF?Zå¼t[O?U"YDU¡?ïäß3'å²?p‰L£Qh?1D]ÊT?;;]·¤3¤?hð£éÄW?n(ܝ›K?ïQ' ‹ƒà?£ýkh=]?_"ñ*Lt?p•É9÷õ?"érª)zF?óë*Î
S?¡±Ò1?cËû†­O?TN K.dˆ?3E
D¾·?‡Î"þ=C?c"—ŸŠôŒ?ïï 'OV?S)‡!?À]?*
`ÈãØ?!1ñ‹ó?^}9|—6?QñH?|r7?ﱫ) ¨?…Y:"U±?Eõ½CQƒ?ZUÒôÉàó?'5ÙÆza<?"/ﵛ´ý?ï½pÊ~¥?':½Ü"%?e:•.{?ž?tó¨Î/?›`ÿG"b?Å©‹âÉO?îÅë÷àKÛ?ƒðª›²i?l¨>éu&?TTø–†j?¡Ö¿ƅ?ƒ§•ß¾¢AGN4FGL J1744.9-1727¿îFºÍ×õÜ@`\÷QÜÀ8ÁD× eÀ;… Äe@ ´©‰¦²\?þú¿"íÚ?ªŒŒk‰?'Ò1n?¬F?Øvd4¾@"8­ñjf?ïò6ci\¿Ü,ûáN2¿äJ¢»Jî¿×a¿â;˜ý'gv¿Å!("-¡¤AGNbcu3FGL J1744.9-17251RXS J174459.5-172640?åAÍ':¬y?¿È5Û¦{Í?p_!uàõ«?aJ…"ï|?Õ:é+clG?¿¦ÂÙÑ9?êIá0Ã(?¼‡iš'+Ö?¯Z—?ƒ¿–¿-ל?ÆÕ]¦4˜Ê?»Â©£Ì	?èö;ÕöÜ?°âϵ¸É?‰ŸT»ælþ?…†ženì?ʍ˜é½Á?°/.ø®*Š?ë‹ö
2ß?›˜b}qÇx?•á1©]k?wZ¤ÑÝ?¾b°\²?˜"‡ì#þX?ׇÍ÷?˜8]6r?ƒ'}ÖÆ#ÿ?v'~5óQ{?ãï"Aµ?«g'荄?âêñXv®?ÈqT¥‡?Œš«'æ—Ý?š‹ò£1?ÙEGöla?Çù!'I?à«ã'yŽ?¹ßUÈUç
?'JÓ¼>Úè?‡AµW+Ç?݃Œtö¬?¹›j®cnÿ?å³çg?±–ûÌUã?ª>%îeɔ?'Ñ=¡€?ÐÚþ,¯û?¯üé ó(MIXED4FGL J1745.1+4731?Ù‰uÏ@>ƒô˜Ã°ÄÀ;T֍?ïÀ<¯l‹C•@º
.k?ýñ%Vѝí?âN.r±M?ÖÄ2I~?ù[4Ú@vkÿØgá?žÖ=
ýn«?ïÿnw¬à¿äY®'3÷S¿Ùv™ºPÉF¿é¢·…<ëC¿ïÿð ¼x—AGNbcu3FGL J1745.4+4721NVSS J174501+473247?";êE?¤"ðú!Æ?r°DQxÏ?|ÎGf??…Îك|g?¡[»ü?ï×ÔUŠÔ?rxŒ—G@Ç?JL#à%?Wyí2ÇM?pÌPÄ÷<ù?l~zÆN?îûkÛeR?'^f™U?z'èë|hn?­S¹m?™î#KÃÿ?ÔL{ŒEý?ï‹"õs›?h‡1€P?g×v[ƒ4?U}·®] ?‡Aºt*€N?e8¥k:‡Ð?ï8åVÜZ´?',ˆyT¸f?"HBœ?›ÍDџ$?~©<õŠÎ?†+áË°™Æ?ï†oŒÐÍ?Ž©Öè)?^ÚãB‡r{?r/rҏZ?Šˆáû ^?‡á!ºÝ-?îO©Å?•z¡µ¥?~phœnY©?qŽ\ã?£\ø^¹q?"I'ÄcÙ?ïÅk&?'Ó³šnz5?i¨»®¡¦?iÜ¥XÑ¿±?šÊEÁ?º†‹aRïAGN4FGL J1745.4-0753?è¹Cá‰Ð×@%£ôË—¦À8ØûíKÈUÀ;ktà |@Ðrá@‰å\ËO?ªŠq¼
•r?†:¯1ƒ?Üùº@®@øìÂ
¦ø?îÃpbhªä?á¨Ü,¼!¿ß¢Ž4ቿâòMà]£I¿áP©ôg¿Î'ÕDÀyWAGNbll3FGL J1745.4-0754TXS 1742-078?èàܶú¨}?»Y€¬Òu?w»çøyZS?gÑ-ÿG–h?˾­ã†*Z?»4u'?í•03z^?²`Šù%—Õ?…r¦N³Â?µÜ—ÜZR?°¨;›R$'?°ˆû§±•?åÀa3?³¸ûU«–?—¤¬f2¶w?'7º¨ô/±?Ó"'s?³މì0?룟Ê`5ö?™W8"Gڅ?¦"÷"˜?ˆ³é?•ª?·Øò⚇?'¤\Þh
?âàºtì¢?ÃŽvóç?'ª¤"N¥?ƒ·¬£T(?Ù%DBO/é?Âùwù†R?éä¾Juf?Ŋ0ÐK)?–W"õÉ«?¤H øjË?Å¢XbÓÆ?ÄíÛBäà?á·;˜²hó?¹b²÷•v•?—U\è^.Ò?o§g>{Ü?Û3LDì?¸ö²ö`9¿?çsmÒ㴒?«;ý¸ü+!?¶ô¶‹¯Û? ­ƒ½V'?Æ·ílªx9?¤@çk?±AGN4FGL J1745.6+3950¿ígO¼Î@=Â!yÀ:ôÿ—$tÀ<¢þ~ö€$@Ú%Oð®@ËÛjõA?ÀTUØ#Âþ¿§ñi~º?é{~h?ý‰J°Rn¿ß?ÒéF€¿æ›#Â|粿àÉÍ©kžµ¿æ[Ù_'F—¿ÔöÜÀµ½¿Øˆ]|\òÊAGNbll3FGL J1745.7+3952B2 1743+39C?îö<¼ˆ?µ­U˜ã¼(?séê?P"F?ÙÁÇ]?œ>P†ø?²"^5z?ïn8sJ5¿?ŽôÜ\ù'?kۆ鳡N?rpʐ+	°?{qýÅÔ?‰VžGSPµ?ï?Y†¦o7?ƒ^óXQ¯?j.°Ã0¼?c
Y;þÜ?"Îù	ݨ?'(_¢d?ï8æ)ÙÜï?ué•.Â\?gÓWFÁ?RN+-?•èÏß<@A?uOCbìæs?îðãMJi8?ŸŒÃ©TÐü?v[•òýp?tý¨''¶/?œL°Ý­ð"?›{=Q#œ?î¬È3q,Ï?¡B
—Œ
?u¾è–S^?£Íà€+\?¢{Ÿ³%?ž'ššû?îˆu7˜%Y?'YýßJp?tth̸ûî?n…"jd÷?¤êm(ƒt?'6ÂÅóûÌ?í,ƽOh?—çk`U" ?ƒÈ›gâ€Ö?uZí?hµž?´&V]E/©?—™iœFŠ8AGN4FGL J1746.8-5235?î€
I¸ŽÀ(v³™õßìÀ9Ågqÿ ÝÀ;ª'°H1È@^+?ô·¢@VF]²c?½—Ù%Ê ?Ï¡G"~Z#@ÔnYyîÙ@Œ>gCÜ?îÞé?Mô¿á]ʶr¿åî€F}¿æI'*K'¿î…ýÉÄÛ¿ïýß1S_AGNbcuPMN J1747-5236?ïÁ'¶(ùý?r4z'±ºÃ?r%'|ŽÊG?hA¯:?j#DÝèn?cÓ(ã¤VÃ?ï±(KE3?—'0žOø?MÅæ-%w?dlTnš?ÙœÒ}Í¡?•(6úé?íìÎ9ßIÒ? [x/?˜ð6ÌT^?'•§÷ŸA ?¥&$C5œµ?˜Â8\c?{C1?nèiD?°?`€2$BÑ?HÙT¶í›?ˆöT'#¶]?mDxÂ>íf?ïkûãT'm?§EŸ:¶?ŠB¬35rº?§,Óa€<j?u|µÙþP?nÀ/=œ??ïJÛ(ÆZ?¡kGp³ÅŠ?d¶E"KY?zx©
œ¤?"
ÒM*°L? ,#kâH¬?쟯£?§æ" 9#?§Úd€Fq?™ÌŸùª\?³5Õáß²?¢Jk¦L<?îgáz%?'_û٣̃?HQWRy?pé	⋉¹?¥K,@~4?ínŽAGN4FGL J1747.1-5453¿Æ™0ŽÏLjÀ*Àaé)#æÀ:=ÀÙyƒzÀ<	¶Å#‹ @Ä>tÎ@²ÔüF7?½g'¬lZ¿ãKX1ß?Î]èHSV@'ß–S"?ïøæ0K!g¿äFÏAò׿èèmÀÍ»¿âMrU€¿ä…áUðÍ¿éï¯OäCâAGNbcuPMN J1747-5450?ïõ-œ£í¹?DDB*l/?-]3±ê?!A¸ÍÐìÿ?RØ
¨?B²\ƒ­?ïß0ö~2F?t¹ã×ÑpÊ?0¯¦"O?:¨@ŸOWÏ?n¹)Ϥ ?søB|ÀZ¥?¡a—¨?~ÑxϽ̎?`<)&ÃüØ?c"ÀG£ðš?†Æ
OzºÒ?zsþ<v÷Û?ﺛ£EP'?X(oxô^'?F#ª™7U?'2	ó:??í¹f÷?W€+Erï?ïí™:p‹¦?S<L©RQ?<Eò‹8I?-½+EïÛ"?]ÅùˆÚ?QdºGl®³?yà¹
?•J_¿²?GÂM¡¥x4?[T¿ÿÀ£?‡<¶E ?"¬º# |?ï:ç¨Mð?Œ^†*ùi=?g›o5ƒ¡¶?f§ÿ¢ßÖÑ?•¯
­Âº?‹ŒÃzò?ï,ø%ë÷à?vÐÚütÿ?bbèûÊ?KP#·?˜¹@@€?vªÚáAGN4FGL J1747.2+4937?Уløb
"@>tºËB‰À;wNÍÃlÒÀ<Ø[¶	;é@!
ì‹?ý²X''†?ËsyŸSAñ? »`=ØS?Տ¤ÐÚN@Ai'^è¿ïÿþÐñ?ïÿ±üfîL¿å5=߉'æ¿Ö3)"89,¿Ùð«C"¢¿Úœå¯ºAGNbllRX J1747.0+4938?ïá®Zy|?j[N|²$¢?-¬vÈh~Á? €?,!æ?mŠjW,Ò?j'¦~®®?ïäÚQ3"?lGÂòŠ?9ɦô	˜£?F(Yÿˆ«•?gìyǶrK?h¥§Ãu?ïWîøàjÓ?Š"Ýø7A‡?Z',NnÎA?feùÜ]å?"Y"vÁ?‰Ôyw6Ú?ïÐÉ7°µ.?V.ïï¡?GÙyQr€?.ú-M/?t¸Hå+Ó??V×ÇN?ïÒv!?rµÏf-?<$ÏguXy?1"#ñŸm<?u/wÈ&µw?qáÌÄ*p#?贈)"k?ª@Œ¶Qù?L)#©—,q?X^<øŒÙ?ƒ]#|õߗ?€IUà2?îãü
ŽU?ô÷"hà¼?d'ðq†è?r{'p? }Àõ#??Ž°OÓ!ܑ?ï{T‡õ4þ?s3·hꫬ?[ΡÍÀt?MÿžÑ|âç?È$%âb?sj~}!Q~AGN4FGL J1747.6-5308?ï·-s€«6À)/ñù¬ÿ¨À:oëBÙÏÀ;ö¶
¨@WS(q
^@~=½Ð°‡?Ä!_÷«¿ˆ†ê%´V?Ãì­è±î@µ›[慱¿í¸®6Ý?ï\£¥¦î¿ç{]U¹¿é6çRŠ¿ÖæÙ¾L×I¿î•¼Ê÷	·AGNbcuPMN J1747-5310?ïÓ+À<	Š?yfR'o"í?5 ªªAW?1~W¨²¦s?uâ+á?y¬èۓ?ïÝÛ	üX+?~NÉ9þ?1ŸM6a_o?Af/&…æ?oñ±¯?}»mùˆ­?îuuçô?ŸCP5Q?u£tþ‡?wg¥Û»5?¬W´=|Û?öÍJ(Ì?ïh7w÷™?oÈ{ÀyÂ?OšŽÇ9Š?;Äç™=C?'ü<¸?o_zqZÀ?ïtÜ·a¼Å?°Òn(Oõú?Ni:mV$?L4'Æ?qB‰"?°Ò$Œ$±¨?ï…zCE­'?§aê¨@U¥?I¢÷ؾ?d"¾çc~?MލÈ?¦À•íÂa?ì'.¤ê@â?§T/PQ[z?" Ññù¦Ð?"!ˆlÊ?¸òp˜•ù×?¥ß9®1?îkm̌5?Š7ßWxhÆ?dÄ¨¼N\?Y¦Çgx®>?¨\ؕzH?‰ðtßµc£AGN4FGL J1747.9+4704¿£µýE™õ@=ù'ÙýÀ;VTÊ\°À<À¿\¢˜@¯d'`—ð@é?^º z?Òu{{vn?ã–]O@	uü wnÌ?ÿ¼–ž½p?ïçÝ>´ñ¿Õ±¥^ɹó¿áÊá:B.¿é™+€À…¿áà‡_rV¿çÈQY•AGNbllB3 1746+470?ïCá÷~?nè[˜?…^–"sÈv?|Œ²tñh?"È8šN•ý?‡ÇÓ™Òë?íh	È;ÿœ?®ƒ_ñWE·?¥·ùÖ+þ?§gˆ2:¦?£Çi¨¾B?™¢²HÇW?ìú!~LX–?¡GRÈ ?¤Õ<5z6?––Ou.?«ˆ«æœXp?–ô]'e?ì2Ö[ìºÔ?"5÷Sv.6?­úwÁ1Ø?Ž"ð}­²?¯ÍŸË*îé?…±:áW'?î
k‰¢?ŸÅùw'æ?–ÆuW¶nh?'׈¥X"?£îžúC¸?•5Ôº?è;CIUß?ÆD'4ªà?´.ʇ'ô?ÃÕ´kƼ?¸¿O\RŸ?°{Ӑ)?ê¥ù'sžn?ªñEՆ¶'?³ûoqà•?£
òhà
º?¶Õ{9]ú?Ÿy&¡CJò?å]³8?ü?«c)
Hª?Âi¬–÷RÝ?©Àõ…×­?È!؜'­2?¡7)#~¤AGN4FGL J1748.0+3403¿íÌ_àÌo@@;-'d2‹À9ä3|‡À<h&£Ø·½@G¨Daª@Öé5¹q?»š¦c'?»'3`)¶]?ûÿ,ëñUB@ã¸cß"¿¦¦²Ü¶¤Â¿æƒ"Ó†û1¿à«Áïùø¿ãs[ýVØT¿ë¬»Ií‰Ü¿áË¡>(¯¢AGNfsrq3FGL J1748.0+3405MG2 J174803+3403?ïÊÊkÉ|¶?mv!4ý"?S<¾ëÔ?Fñ?	2Ž?u˚y9¼?j—¶XTÊ?ïÕB?s;?s|Õöç‡t?N#µoHw?X°rîóßÔ?qši˜3ß?mE±a?ïjõˍv?‰d'R‡Ê*?|LöƒaŽ?Î¬¬Œ©?‡VG=ýˆ?'—ˆï­x?ïÈï(l?WÔü¦5q?`VÔ0š?@þVw?s›ý³pÙ?SÚMCŒú?ïsW†¥?…ƒÍV>ãÜ?lcº¸×t?`E±q.?Œ&
Í÷Xâ?ƒ'>*b ?ï–æ£SŠ?‡¢P&§íA?Xºk4ýâ?h¿Äe?‡/-¼'A?"m¾
?ï •&B^õ?'	,û"š?€Æ^Ä?ƒÝ¯ø""?"äx'=}?Š'Ð¥Þò?ïcb-¥2]?w˲éó;?uwø @ôÞ?]Ñ+1)>M?Œkx†êäg?sT"Ì.AGN4FGL J1748.1+2702¿¢‰=AY/ª@9‹¬q³À:Ð	sFHºÀ<~Êl <@"êƒÁëó@­[î=`?¿ûòTEÒr¿¥QÑìqX?çÛBEõ­—@F´\"~Ϳ蝘—;ˆ¿ãƒ¤?9ü¦¿è–Òª\_|¿â'¬¸ZO¿×™ŒÃó4k¿àÓ¸^€¾×AGNbcu3FGL J1748.0+270187GB 174618.6+270457?ïæ2xðy?VïØ\yZæ?@ŽO§z?0Ñ^§M£D?e©ó#¿o?Tic®¬?ïÞ?uƒ1E?j¨KA&¥Ù?>‡ÙØjç?H–{4ç±?mïSŸVH?fёÉfÉâ?ï®q—i`
?tè܇³È¯?RƒIrE†?TUÕíƒa?'1€æ?tZËeŠœ?ïÐSšSJ?U‹#®?>C*›¬?$'yëÂ<9?v
#¦6®½?U€»,ãw,?ïȳÏ7?lwäy¤ú%?Pƒüú?Af›å)2$?wº}Ã8õ ?j¬q
Œ?ï–bsÎÀ?…'Ÿdyl?Pº]¨‹²?\¡æ¹ôŠ?ˆc›¾‰~t?"
ÅßtyŒ?ïk?S§òÎ?7áS¦ ?\hš_Ž?Y=®I?Öÿ?um?~#Vc:j;?ïY³•÷¬'?wú aÿ¬?[=¸c½?LR£[=LJ?"¼QjÛà?wÀFˆx՗AGN4FGL J1748.5-0854?×^ÞutSí@#O27Š°ÉÀ:…#\%šÄÀ;ݐZU¶ì@!Ÿ¦HÈF@—:*?ÃIƒ—#ȇ¿ŸŽr@†¥C?à‡ˆàcØm@^ô¶uÈY?ï"ùV˜"	¿æÐC¿dT¿ë4tF"ú¿Ó§;cƒ¾¿ãºua«ì'?Å/D%ɾ%AGNbcuNVSS J174838-085435?èX±#ì«?Àç¿ÿ×3?rÝðuCZ?g/¿	¼~?ÎKð)¯b?Àá+øñØ?äô(Òޞ?ɋÆ첊?æÙà¨ï?"´ã9/R|?ÕíºÇÖ?ÈÕV˶Î?ë,Òrvw?¨&?H¯
3?Œq³œ[2.?"s'U{?Á…šý$Œ?§2Oò&eª?ëÈìöìcŸ?›»†°1+^?|œîØLG?cÇòò_Ö?¿÷ŽyLi‡?›''_js¼?âÞ~¢¿ªr?ÇV‰¤?ÿ`?¿3?t¯^®]_O?Ù³	Æìý´?Æ÷Âø@K¨?ÚxÍ"wÇ?Éþ¬¡fË?'¤¤Ÿ
C?š!ooH2?â6tR¯œ³?ÈÑ7tz??åM܀¸»ã?³‰sãæT?—€bý*—?ŒqgÿXp?Óì@΄æb?³$8˹×q?ã«õWÁ™#?±U±¾L®?•¥~œkš©?‰yFÆk'?×M½fí
Ï?±œS%tŒMMIXED4FGL J1748.6+7005?ïÿÏ(FÆ
@>¶–¢nTqÀ7×m̌5À;s;BÌ-k@ðˎkß?ÿ>(	3…i?–PÕZîu?¨Œã¨±d'@'
¹t*@-…Æ}þ¿•nZ·Â¶¿ÚëèÜLòw¿áaÚ«¿ÝóÂo{¸Þ¿ãO¡ÓÏË¿âäî—!ðAGNbll3FGL J1748.6+7005S4 1749+70?ïó'y±ê?F™W™œhÑ?3ÿ]¤Ï«?/HÑõ:ˆ?Tªëøø?Bþ¾šG?ïÐóG—?söyÅo£?Jl¬òÕ°?S_Ú
+§n?t®pËÚˆ?qÒz#ó%W?ÓnÛ?†þ8`¶Òy?mâ'Êã&¢?~…#!a‰?'¦¸o¬c?'$Ž-–mk?ïñ³À¦¼?Ah⠛@P?0Jæ{hZ? 1y\?X…Å(Ìþz?@	\卺W?ïìáۍì?V× 5ÉX?2‡]î!û
?/Ìùa†H?aŸ2TÏÜÀ?Ui
׳©e?ïˆm_[°?Œ¿"Á™ˆ•?`‰sÙÛñà?l'Ö3ûV?‰ÂC>À›k?Š0KNm×?ï®×
Oz?'ZœcºmÜ?eÿ,n¾'°?wQ©¦õä?}"äæ5‰é?}¯{ha)o?ïãZ%÷q¢?[n'":~Z?>"ƒ³Í<š?1vÌï±?hÓi"±6ö?YÌpŠAGN4FGL J1749.0-2327?×8§9t@­¯ÑƒÀ9"¸'ú
À:©"ðÅÐY@÷i¼‡/_@KUhè!?Û¬kBïó?à›q«>Ì@GŠLáZ@ñ҆õýô?îíN·ó÷´¿à*èÁŸòú¿ëÝõéüˆ|¿îç}R;6¿Ð6'Τ=b¿âGß½•LAGNbcuNVSS J174940-232619?ÐúÙs?Ä]~ÖtÁH?Á?@T%h'?¾NšËP~{?ã2Ã1v"O?Èèo­z2?Ú`HèÚ¨
?ÍÃCÆ?Ñ?¶tµ»¦C?·8Ë\¤	¤?àYôèõ¢?Ë~§Î™3K?Õ£¢0ïB?²E@jU¿?Ė´É)÷?¯ºî²]‡[?àµ»ýá?³®Üûþ?Îa¬,ï!`?ª)|Ê,¾¸?³iY"wÊ? =îÁ÷Ù?æÉրÞ?­72ÿÙ*?ʺ""êõ?ÀÉO®'Ζ?ÃÙð#
"y?Àì:VÏ*Ü?äZÞÒw d?ȓÚ"uØ?Æød^?Ægáʤ˜??Å8Svr?ÅD•Y ¶7?å-$µäJd?Éy©D•?Î?\28ã?±Uz¥2‹
?Çé˜w' M?²"s°"ˆp?âuÂÖ:?µÈâhõŸÅ?°(Zñuö?—ÜòôN§ö?µwt@±°n?®E
!^?ëLäF€?®nÒ
öîOTHER4FGL J1749.0+4321?ëÜoxo
»@=&éÝ~˸À9:ªö¹/aÀ</ë/³L@j©t@lŠ½]Ä?¨–ºÒ܏?¡§¯†ëÂ?õ꾅m@"ý™É?O?ʞΌÀmC¿â4¤ý¥Ý ¿â‰ôafL¿à"IÁj"¿ã%"R¿à–[@î\¿AGNbll3FGL J1749.1+4322B3 1747+433?ïñùæqŸ¼?PRQîçó?5Bþjœ1?)ÅKÿ7ŠÅ?VÆ"ÞW0å?K'âÏ\©P?ïÙÜÜ©'›?p&o'h_?FK`h{,Õ?R4q:A§»?pH%­i}C?jcåþÁ£?ïÆpN
"Ç?kqœÎKÖ?P±Œëcxd?8ïÌ/8œš?x›u§ÏúÃ?jbÕe·9Ê?ïÄMs•ä?Z¢ØJ–Š?c‡‹FîT?E€n@?t€ŒV¶Ø?Su ±‰üù?ïçöï` ?[Q3Ü?Bݏ&—V?6CaÖ?d@¥#ûD?W Ù-ËÆ?ï"SWÒ
?‡4—¸ùK?]*¡×ê+ê?iå0G¥Ãå?‡YÖ⯠?ƒ­àÚÀX?c&Ú?zL€Ñ<™G?W?V®™x?D8àìVì?…+DLA>g?y¨ñ¢?ïs«6¶0º?s´j8ٔt?wshØ[¡;?`')&úž¢?‡[}ßfÈÛ?l² £éq¦AGN4FGL J1751.5+0938¿îyv¹oÎ@1¦»#WÀ7ÃãiÇC÷À;PáK	Î@ ‰ôµôï@'òeÊ?šã[üÍgõ?¹^Þ¡zRp@;'—•@F]	pl¿Ç'*t¿ÜmùÞýQ¿ãØÊfÀÿ9¿ãçހÔPпçL¢Ûa»¿èMÄC'OHAGNbll3FGL J1751.5+0939OT 081?ïڝ•\?eqñ¥Ð?LHYȌ¸î?Fä_j+y?nPä=¾'Ë?bfx>Þí¡?ï´þPJ×?¥J§ÃþÈ?Z#N•'?dƒ¸CG?~ø#*è?€Mwu	?ï®hÄ˲­?ƒL¯h0hš?q§Féèù>?}à±X¥'?w$V£/,"?wÙà?ïÒäÿÒa?\òjޕÖ?Jù˱Ëüi?:‡'‰ÑñÓ?s.F¬è!?Y'á`sƒh?ïÐDÖ@5r?pð¿£ÍÙ?F)BE¬%ó?AwNͅ?ulŠÑ*"?pK9¦H5?ïEN ™_"?œ¾ì…é?mô½þA©?÷'fÏÓJ?"—ªíY(H?—zä\<j4?ïžanÒ=?…Ÿî¿³+3?qµܛB¯?{Ñ4 %1æ?;¿Åƒ?'s' aö?ïŒtõö;Ü?yºK¬+
¨?`|¬eY(?R\ÍNk¸?ˆÃ—m:-2?xÇl÷UAGN4FGL J1751.6+2921¿ÚO=æÛí@9†¹ÃÀ9øzYbqåÀ<÷­K'F@Ÿ6²Á@™WÚ²h?¾ólɬÜÂ?À½oø
",?þ7Ó
ÔoX@3Žk¾"?åÞ¥µ%ç¿â"Px¿è=AÞËÓ¿çþ~pHg¿ë>¥Œìâí¿ïù‡ÀÔ AGNbcuMG2 J175143+2921?ïô®W?C¼½Áß)?>öŸ'õ^?1¬ÕûèuÍ?M̞yòØ´?>I®_Ò`?ïäßÓÿ?k&÷'J®c?=$µB'x?Hí&ƙ?g|[UÉ-¯?fªÙæq?ïºvøž¦Ž?kº'ñ?[cö-Éê?Ge/Úa6?{ë†0"?i·	Í8?ï氏^Ð?Gtß±œã?DØ	e(vØ?(©Rèu}u?dÝýÆǪ?EÉ®ä5¸Ò?ïìÑðM0?U	sZŽk'?P&ǜYÞ(?F,®°&?WÁ"=ÆÖZ?LHn(¢?ï°PÈÍí<?ƒÝܝÜì?P'‹õ*f?`dó!M/?æÜ\P§§?ú<EýL‰?ï}F¦ßè?}	%®;m?h°î1Üº?c´½$KÙY?Š'ö<×?x ŸvÃä?ï­nù'Í?nIêç`h?aޖUŽ?M²÷Û6§?€,œy5%?ke[µsŽAGN4FGL J1751.6-1750¿æ®†f@?éúÚýÀ9¤±ÓLBÏÀ;t<"¸@ ,šä"@¦ÐNaŒã?¾&—Ÿ-¾? […â­‰¼?ål"¹™@׏SD ™¿ïƀW~A?ï÷a–5¿åZWBÖ>¿ä
º}¿ÉY¿â"ö¥
k#¿×Ïî,ëñAGNbcuNVSS J175120-175112?æ&°æ½8Û?¼
ɋéq?wÖ5iãÛG?h¼ßöžx?ÓSE]"j<?»ÿ(¿'ÐÍ?è@'÷`k?»-ã
èJ?†æã;ˆž?ˆd9´ƒ_-?͏Eî Úk?ºVbžk÷†?åtý]c]r?±Ã꓃ÁE?•1P<Õß ?‰6½UU?ÓÂðA¾]Á?±£¸q$?éu¡_
Ò?™õBØYØ??•ž=búÅ?tyÍUcÛ?ÇxÏ{?˜ðª‡DÜ?ÞYxïLuò?Á¼ÐÓö?"Ø,£ãN¸?ÉR¬»®n?à,'#-²?ÁþÐ!Z?ßÁ¹z×Ùé?ņz¥ZŒ?˜íÚTç?¨ÁŠšëVº?Þ¯hßx²*?Äp²ôÎ7u?ڌº)a­?·aiòP?¤º5rÜ?'M¶?vö?ámú÷Øi8?¶¢`©ÃEU?â'X@?¨Ÿg‰³ä?¦Ûè/ÀG?3zÀ`cà?ØdãsF8?§ç»ÛJÚhMIXED4FGL J1752.1+4531¿ïë薁â@=Îg×®À;%3BEÀ<†#mÃQú@Çkcü@¨> N¿?ËÀ#8?²šð €Wm?ä^¯¨Ï˜@ø&¼x{?ïþ°_-âç¿Ì7ªçݑ¿ëênió9¿Üc—¿yÓ¿ïh¿ëxá=G3AGNbcuB3 1751+455A?îþKÙá÷ñ?ª¸4ùש?s(ýÆ.	?€c«ƒ?›lETq<?§Yú±WR?ïJ)·çëë?·ÅtU÷µ?xe"õБ?{Zp©SR?¡ƒe(7|?†2_!k–?î¹ü̪ú?››­^â'l?ŠDWåóy?‡úG†Ðë?©#J7$½ ?˜sçTù±¦?îâúª;än?zæî֞È?Š@†óÌ+?lC'nWô0?–€¡øy()?s"­—Þô?ï/¥£×ÏÏ?˜ïÆ -Ÿ…?qÎ~¸Í¨s?s}ÃO¢Œ?•—«ß•œø?–kgAs6?î@í_á´]?¦1¥"ÅC?‡Îüͧ…n?]ý¬Öœ¶?¥ýjËç#Ú? [Ï{×%'?ìúYßvü?¢=–Ç(ß?"Õ`«L°™?@iò05?²÷ÞÔyMü? K=\€)H?솼±u?š*kmª?¤â€5'?É´n¦º?±XÚ.™¢Q?'$#à #AGN4FGL J1752.2-3002¿³—áðM¿üøÉZQ….À9]ʊÓ-9À:""д¸Ú@f­éê*@RaœÓ
?ҋ$÷0M¦?Ô½ÝüJô?ÿ€|¬ùÈ®@LH6z?¿_&¿ë¢AsgÖ©¿ç¾BuE|¿êY`úÛ4¿ïís 3*?ïH™"º]AGNbcuNVSS J175230-300107?æ:±S
‡í?Å'kB²ñÉ?¸|Еl)?¶VgÏHÝQ?Ë	üKH0y?¦»"ꤾ?̚$eÝKí?Å.~èJr?¦qˆꅞ?¥Ôa?çr^eLF;?ÄÙLþǁð?ÙzŠò÷?¶‹}Ô}V?Ãà¶{A?¬•'ÇeÇ¿?ܕ¦¯E—(?µ
•µÀ^?Á˜¢àô? •Y!D?²#LJý,?—ü¤^w7?és¡ª¡Ý?¥ˆ³õx"?âì,
¥?Åi¨S/'?¾—È^()?¹‹¶Qí%?Ô`<4}yí?Äãij×;?µÁ@4u?²ñ¢‡8tå?ª¬vq£?°eŒÙe?띘ÃI°?·¾bþ\NÑ?Î'—dœH?°_g°È.?È'ÁŲ§2?°®6w¯?âl)µlD2?µ ±·Ø?šXBِÌä?"eˆ:¹žÏ?·¯G!õ?©Í²_j?ì7U.×É?ªæS.áMIXED4FGL J1752.6-1010¿ÎË÷¯úY@ K›ˆ‡"ŸÀ9Íj'E'À;rèn@P(Ð	˜@C@ˆÊ>?Îľ ¹?Ú &5j@Ž"mR?ÿ¨]—4åe¿æ½8:1
?îß®áÕG›¿áÙaÏ©¿é…V`߾¿äõ³;+¿ß«©f–7AGNbcuMRC 1749-101?ܕtè—A?Áï¼dš?4±»ãì/?"pòZÐt?á8rÅã?Â#nƒ¸K?ገºÏ+?Éeû"£?Â	¿U"°˜?¼ûgrˆ'?Óâà:	^?ÃOt3¥ì0?àx'Y
]?±°ŽYËÅ?²ü¬ž·™?#nIR½?Û¯­¾?°ïj0 [Ö?á~•-'ú?¢OâŠ\…?»î>Pa†?'t·:}û?ÖFÁªk?¡?l,´?Éñ¹1J¶ï?·v}^T¤?ŸèŸ…#½`?–ÇË»g»?è"L·­o©?¹ÜÔ!¦Õ?ÔÏ%"H­Õ?ɼUċ=i?Р¤˜Ù´?ǟ²š=û±?Ún¹Èxw?Ȝ®™RnY?Ôِ`q'?°Ä6Ïh?¹i«	â?¢
Æ<Ù&?âpŠ¬–Ì`?²HÌ=)?Òë±ûv?¢Ã½r?ĝ	nFbC?¤ß‹»;~&?á×7.•i´?¨ÓHkB‡ÿMIXED4FGL J1753.3-3325?Úû|Ë`DÀ
ÐãF¶žÀ9¡Åè¬ý$À;–÷z€Ï@F³ÓÃt@uêgèG?ā¨÷…ˆ?âç@Áf<@w–¿Ê…Ë?ëX{-a¦Ó¿äBxùæá?ïøkç¿à	'Ë û"¿çM}™ù¿ïDÀ
¡©?ν{¶"¶ÞAGNbcu3FGL J1754.0-3321NVSS J175308-332637?j¬.7D?«X¾QÅ?ç¯]õñq?ɽH"lûp?Ï52¥!j¼?ÈüËHÏc?ŸC¿L¥'Ø?­iGÚ­?ä,¤9õ]ÿ?Âð‹õ'p?Õ²{—ò?ÁéQnBäè?ºy‹O\'0?£¯¹Á'@â?ã1?ó,\?µˆgZ;½?ÒÿEÏÜ»?²à‰¤d?¤¿¦OˆÊ?€Ó2,Nà?æꕣÑçû?§áº´`35?Ï%¿Üh:?¦¼:û~\?€§él®g§?z`JŒxñD?èvHšOd?ÅiÔÚã:ø?Í_ÿDÕ?Å,.[8?.,9ú	·?¥OþEÝ?äËØQv{n?È]e…Yµm?Õel™Žåi?Çí|+÷?©æÓ,dh?—q£_?ä³,g¼þ?·²ç?(£?ԋ¿AÚü÷?µç–´…ñ?†µk\Dy'?lƒ‹8ûm£?ç馳ø.i?°º(€î'?ÎîyH?°h¶ÏiÈPSR4FGL J1753.6-5014¿ïH¯p4_GÀ(3¿ÂÀ9q¾íæøÈÀ;ÈLáZ"‹@™Ìs™@:œ£9V?·íÍ9Ú?лWYƒ)@ó ÔƖ@@Ÿ7=Xü?ïôT›bÇu¿áÔX<×ø¿æëªÞe{…¿é
áSíh¿î?S‹˜¿ïþ7=ƒï
AGNbcu3FGL J1753.5-5010PMN J1753-5015?ìîÓqEX?´â5HD
?¬
—3·V?¨ÕˆßÂZÉ?¥1»`!?¥¿š1µ}Ò?ïË£Pîâ?|·hg¢á?KDAûÂÿ	?WžAHȏ\?vÅÏÚ'¼"?z f1v;d?í"Y7÷	¯?£7PؘY"?¢Mµ?™Ï<é•Zp?¤lÜk3&^?™8få¥&?øô6ã?l^øiûʦ?g"ZF=>3?Ny7•r"6?‰	+8B/³?i=ÔÆ,?ìÒH(Ûù?²I‰Ø»«X?©.2ǗGŸ?¢ö]iè|?©­J¦leÚ?©Q3õâ!?ïo(1Õî'?œžÀJ‹?a'ûêkt?q¥oØÙ_'?Ñt"`üm?›J–ÈÃy?ì ÊkÚªÂ?¦êÍ/FŠ@?­ã4Äg?ž*[e"Óµ?°=X¿?Ÿò^"¦cÙ?î4®]uý?Ž/wÇÓy?ƒ$#1·î?p5`*ÖL?£C¬QR2?Š§ääZWñAGN4FGL J1753.7+2847¿çþÀ묌@8tH@árÀ:écO͞À<SuDO»)@'°
ú> @Ü@Þ¡,?ÍÎ#äᖈ?ÁPý¢}C?ô'À®9@¾·ëêl¿ï¨"¾é_U?í4nfåè'¿æÍöÎ(Ÿ¿ÜI¹à<¿å'¶þ.o¿ïÿnªØ†>AGNfsrqB2 1751+28?ïچ‰Ð'?cóqíÿ0?N=U)ý>È?E¯‡iÊ+?mê ɼà?`xAó`z?ïÕ
©&T?q-ftá?IÆh9VŸ?Q"*Ê>Š"?r<­¼°"Ì?lµ7QGh?ïŒ[š§Øï?|RÌ[ÝÔ6?džÈU5eä?lð߁}i?‡Ág5e´Ý?v‹Už?ïˆOxtl?gÕQO+Î?dýÆ'3Ñ	?H [Xù?ˆ¬°S˜¤?d®ÀâNº[?ï¢(©
ø3?ƒž"+ûÄM?eí´ýŽè¼?}ÎÌ,oï?úhrÏe6?v7²þSZV?ä¶oá?…4ò«!º?Y€9҉?a@÷{&õ?ŠröΛ1‰?ƒAšºþX?ï½)/"?‹oN:¢G¦?rú¦ŠOó?vqEp'3?—‰±;™*«?‡^J$l?î´+J?"áÊB«a?{#?=4@]?dèwqR]?¡YÆÖÍN?ƒ*£îåWAGN4FGL J1754.2+3212?Ø"Ÿíƒ@9hÇ\Jƒ²À8|'¿bÀ;'=mHØ·@üµ‡‹Ð?û÷BÖ>f?¤v3ãÝ4¤?ºüYxûê@'V†''@°Ž'ºR?èÄHÏ|ªv¿ÜØP÷¬¿ÖL˜_¿ÜšäN¿ääúœ>¿à#Ü~¸AGNbll3FGL J1754.1+3212RX J1754.1+3212?ïñ;oÓÞ ?Læ–LAºƒ?:߬!Ƽ'?2®y:€Æ?VÑ5Qâ™?Hæ®Õø?ïÕÝ›ß<?q}ìã@HD?MNv¶0o?Z7«÷?ì?qg®¤;ˆÀ?lÜû,o?ï‰+Ó¡û?Ybž?|s_!¾`·?‡þýAKß-?~ö·%Ìeo?€mÂ"<Q}?ïÎ.ú>u?[ÎCÌàÒ>?Bâ­­yí?-3¼n»ç?vŒ-I^»?Yò—}ÝÀÙ?ïìn,8å?VRiOÁ´?5)Râ¦óJ?)­£B"<?`ì¾jðu?TÖr€¹˜y?ï‡F+,§?ŒN-:rË?a™/L¯í)?pÛÖIË?‰È)o¨?‰HS[ÓÚ?ïŒÛýä"6?Š?0ÝÊI?tί)"—5?€õùHƒ4ÿ?'a¨íA²ã?'õÚ~cw½?ï'ØÎÍ?uÖg²l%z?QTÂí!ï?>}q«'æ?‰_KñÄH²?u?>ˆsÄAGN4FGL J1754.5-6425¿çwck+ÙÀ2yhÍJ¡À:÷È#àÀ<:©€—j@bÕ~w)W@B:73s?ºŽ4`¯Ã'?ºOM:ö?þ,—£TY@›ºø9;¿Õ6³t¿àTΎmìm¿æ²2í"ò¿æ/
¯†k¿ç¾;]e¿ä1RB˜AGNbll3FGL J1754.3-6424PMN J1754-6423?ï´ÏkžÅº?rɾ,ãR?MAI~™ƒ??°'?€ø"žì?qñ£~œS?ï"ÍÉ´?‹¥gIG[?f•ÀÓ»šž?p{—#ÀH?…'KQÎ!?†c¶×ĬÖ?ïP¯TÓ¾?$Øu¤&M?lâpßyjU?e¼‹`l¹?'MÇ\k'ü?}ªV+?î÷¨_t?r—TtÒ??€nϱ¥ŸL?X'å	yÒ?˜ÓŒD÷tÏ?púzpc´=?îý±ÉèŸ?'òÇ}Èý?hTpUŸ?\ÈR2¬??N€ˆÔå?'8^¶Ü¯ö?Ԩýÿ?¤$ºôƒB?Ž(üëNö?"Ä
á:?¡m•"Ê,?¡{‡gãT?î
e<Ml?™äáèÿ¯?…þøv§YÔ?€£êWƒ"Ù?¨¯›Ž'RÎ?•å<ŠhÜà?ìÕƧ*?"F_ƒõ͵?™å5'{A?}I³ˆ1?²ÝüˆYÞÌ?'ÂB9žLÖAGN4FGL J1754.7+3444¿æÅx'®‹@:
~À¨À:ÉÕTZËÀ<YT¹•¸@Q]f¸pÊ@Ð_ÿD^?Éþ¬˜ÏÅ%?Öèè÷¥¾k@×èÚI@¨þoÝ­?È+Ê^2K¿Îy™ßd©ù¿æ¬¾´ .¿ëOÀ²0¿ð?ìçìãÉWAGNbcuMG2 J175448+3442?ïӄú{0Î?š¢ºó?c†xŒ
?w"*(	?hôYe1?sj1¤L+?ï+qÈÅ+?‹qæN?i֜¦(´?u5䂑æU?'?|‡…?ƒM/z˜TÒ?îLÆ·ßÕ¾?›ko{Vñ?"Böfýy¹?'{0–Ùr?¡'Qóƒ>?"'»IÄh?ïÊĞÍW"?^éõb|Q?TÔºô\…?="Vß³n?u—;^8%?Z7W†ÙáN?ïÓH<W ?t>ç6O†G?Z&E†h?av|ŒÚÇ?oµ°†ß~?pá »Ä3C?–<d?¢·N×Æ©\?yOL*½NC?M/ö)z?–›öÉoè?šfÕxÍ.7?íåB"¡? ;¨¡Å@?"%j*'¼
?¶šA›g
?§›ÖÉpŽî?š`®^ø‰?ï+»ˆÄ?ƒ|Å(¸¹?r¤`ˆ[!Ç?aÑ	R#5R?•óðký?€íõ"ëAGN4FGL J1756.3+5522¿Íׂ©Ž@=¶ê šª;À:€~?¡À<e–È.›@ a®.ß<?ü6À5¯å?¶oçnŽ¨û?±3nÂUz†?ûgÿÚ$@æ~ÜÿÊÑ¿ÉîRCÙk¿ä s"6‹­¿ã€í0£?¿Á5µÙì¿ßÖ÷¿àÏ>šõ9AGNbll3FGL J1756.3+5523RX J1756.1+5522?ïñ{6›â8?H-ÞGë?2½bt·?"r[ït1R?XZR1R>Û?EÌü)ª?ïÞmO¨xž?oÓ.)Jßr?Eß](}?O½!»u?lÙ=Õã?i¡x·×O?ïÀˆ^fp?g°Â'lR?P³nö@`?7@'<.º?{º
úÓ?f–èے_®?ï…×y	gn?c«â˜¥K©?dv±L'¤Ž?DLVg²cZ?‰lu_'»i?bP¹{K?ïækõÛ?Uà1ŒRô?Agâd(?.e7‹ü¡5?e1:ô"v?Sî&dç?
2o?…®(j¨!?Vo…S¦m*?bM>î?‡KUì¨?ƒ
_oÐN?4ôJâ?s»Ùž*@?X+)"ßæ?G½ËpɀË?ˆ×͌f¹?rRîÉӜj?î²siHï?'.	¢pû¼?|¾Ô'm?da¥"˜?¡AÕ^B?€Ás£ËכAGN4FGL J1756.6+1553¿ê;"´Ñ.@3PÅë1<À;ۉ(2NÀ<†@Š3Ë	@!M•¨H^@&IlÊ.?ßËƽi,"?î'­ù¢î­@ñ'À8iÔ@i@e˶Í?ïþ@Bo	¿ïü­?"¾¹?ï‹4|¿·^koe¿ääc1Ù¿æ<ÞÏ®©AGNfsrqPKS 1754+159?îÓÂ.…›Ø? R `ÏÆ?oJ³Ç1E?¼úT–ñy? Ï1×ÔÍ?Þ֖xr›?ê¦Wª/?ŖÖ#kH?·y¥†?»tÜ`h }?³½{-˜'?µxŒºªƒ?í÷X@?žÒÔ›¦?‡-`R©"Ä?†,:¬µfe?ªºÒc	›§?›âÈÈÂbL?åօû­
?³Ò fÛ^é?¹pB<£e?¦ü­‰<^"?Ëß/ñ	m?²FNIãD?í‰êÎÚ1ÿ?«×ÖÁañ?z€%p"5?x£€±>ô?²§0•zú?«ûL'n?ä‹z"h#Í?Ñ	-HÁ•?Ë.ÿID<?Îy~g9?£eG,?Á;Üô¸?ìeŒåè7ó?¤W;N€Xº?›°Y«kI?p!*fÖ?¸¬¬¹år?¢ºÍÆÇÐ?×v·þ'?ÀŠâéç?Æ"äž,©?¾oï‰Æ»?ÝwÊøóWŒ?µšùbyiMIXED4FGL J1756.9+1531¿îÇú˜7ñ@2æãæÄŗÀ:ðHG—nFÀ<b.bT@»ÃZ]C¨?þ³(fP–ñ?Ôào Ê$ý?Ñ¥7<WI=?ÿZÐeށ*@lÏ,M'?ïn+÷Տ?íû.t‡'Y¿ìp2˜Á?º °º›í¿ïÿÖ_Æ	?ïú2–UA{AGNbcu3FGL J1757.1+153387GB 175437.6+153548?ï%ˆ¥«v?–'Ä÷·C?"Ï®€:àÂ?"ŽW÷+ÓÀ?""w§½"ì?'lOW­Æ?ïò´¬´B?§Ø%ðH‹?€cö¹ù(?ˆg›ü'¥?"ï®	ya§?¥Û#ÿBþž?î2Y¢i?šg>C*Ï?ŽÜ½kìôF?‹B\'7Z?¦Õ«›ŠY?•…?✁{?îeV¤…?Šz¹Â,`?‡óN2€?w%fæ™Ê'?¡,翗Z$?…ÎôŒ‡Ìã?îOÐê,Ý?¥ø…ȍj:?˜Œ²#ªßO?ž×šPæ±×?y0'™û&?›.aÄ‹e?íÎÞ¯o¼?¶f9Dð?—aVf{ûr?¯Ø³½Š¤.?§aiÓ2‹{?¥×§ËzV!?ìr˜È۝í?¢¢´è'õc?—ÄFoºž?ê™å~r?¶z1é¬ãk?¡&Œ~?ëæ•Lq·l?¦x¼t"V?Ÿµ<}Øʑ?˜Ú4®!TÓ?¸Þ~³ßø?¢;ÍîWXyAGN4FGL J1757.0+7032?ì·L¥þŠh@=ù…H©¼ýÀ;‹y¢ƒÀ<©ô§Ý);@!· ê±9H?ûI>‡û¤?ɳû*-P?¸4tѹ?ðK'ëk:@‰LC$—å¿ïêKÎ4«Ù¿ï']Àz"?︶•Râü¿Ø˜±ý""¿Ý/<Ùz/¿ÖAW›:ÙAGNbll3FGL J1756.9+7032MS 1757.7+7034?ïç|)àèÒ?YXŒisvÆ?-TŸ‹–a¯?t•@v7l?f®ŒGZb?X~>ˆŸ î?ïÖv/ö×|?tÃCn7=Ë?E
'ÏÖ¸?Pj·L"œ¢?r#DßHF‹?qÜZ'·'?ï]¨ýGå?‡Iö¯yt?Pä‰Ã?CZRàè?"<—Ï®Ã;?‡WAP'?ï‹(µÞ?mݪƒ_e'?Gç**–0?:4í=Ž!û?‹¼ÃMÍÜ?m‡eä²-ü?ïÍJGï$]?jà¼7$z?8
ÂFVÐ%?)Rðß:?wÚFÇô?j`
Ëáe™?ï†0—ç+¸?ÞŸß¹ Ž?YöÁ…vm?gM'ۍ=?‹R[5"‡G?ŒJ¹`%ù?îÁœ¨ PK?•@@'"(ó?UWµÏY­?X¬x±|N?£;wÑ"?•''ÞG1?îÊY"8y?ŠTõÄ þ?VF÷Ý[9?SÀJ_Ô?¢¨6$A(?‰þ6ÓÛò AGN4FGL J1758.2+6532?âi ç…y–@=ý)WÉÀ;K³ò
s÷À<¿ÇòrxÃ@ûX4õU,@åùÄ|œ?ՑBq>²?Ú*–ÁøÞN?ëáÉ^-\Ú@¬Ô=Y|É¿ìA#`Ø2¿Ó‹ûKeY ¿ä×	 åþ¢¿æjK˜"Ƥ¿éK§ž?¿Ïž¹(«õAGNbcu3FGL J1757.4+65367C 1757+6536?ïH‰sS+C?‡Ja†ÑÃ?uÔ㱉?fN"»œ¿?'yÑHØL?"Z"=ö
l?ï|'Æ׍?Š°oꋴ?o…£ê좟?uMötè<›?‰ÏÑ×&,?'l~xÓg?îd•äa`?•™Î*—n¡?Œ7†vsœ&?…ï;¦cp?¢¨Í•ÔÐî?'~ƒN?Þ?K5wJ?cŸ¡z~v?p°«…QO?P:­W7H?ƒÃlLã?_–÷!ºÝÝ?îP_œ{T? a("›•#?‹ëÜ3Qy
?€N¦¦§?¨Ð÷¬?œòÑvÞ6_?î…þ9¬I?§3÷ÕïH=?…A¶9Ւ-?"P0 Ú÷?¢^RŽË½â? ýšz30?ìæŔҾ?£.âãÝ?›nOtú?'†3«ì?±éwÇDŸ-?ôáü¥P´?î«ÿò¶bÊ?…y@4'Ñr?ƒì¤uÄ?pWùìÑS? D׶ºÛ–?ƒt'{AAGN4FGL J1758.3+1429¿êôãaJå@2.ä¬yÀ:'¶ªK˜…À<>­j0öB@®­€VQ›@ÍæÝð
¿?ʞÌßAC—?ÊÑJµÛČ@t¡'Œ_@dlH¨W?ïOÇão?ïþ"û¥'l¿âݸ½vB§¿ákßj‰6¿âøÀ$óª¿ïü;±îAGNbcu87GB 175603.3+143022?îi.˜ØT?¶@= Hª&?‹hfP(ýÉ?¯6Jt*dÒ?¢"Ö³¾N?°33€ð\G?îôÔʋî¥?—ôì?r u?…"ÀÞÒ¿È?‡º#uý'z?–Ô89"†?ìЌðŸØ?îÀ‹:?'ÂÕìÊÝÎ?†ßé'I'?"K/4Ò?œº_þî?‰PüCsL?íà ûHò?¤Ÿ˜Gp=? Š,g‡»°?ƒ"«l%ý?¯GɈõ+?†½òii{?íg… vÿ!?·è*{¬X?£§GW,?·Íó‰?¦v¯d?š[çÑBÏÊ?íss{^?³X$Ä°s¦?Òu>#/?¢z}œt&?°wÄ‹¬²?«Êzlj§ã?ìË·ÈrŽØ?¢xŠá]&? /:È"/?•)ßÈ3'M?±Š¤¸ã_+?œ	êÕ?èã9zŽÖ?¥?·lf¦??²yÂÙkÝ?›#»Å ?Ã7®;½?Ÿ›•bÌT·AGN4FGL J1758.3-3028?ïÛΘE À	VDÿäQÀ9‡¨ÖMÀ;$Y'¹'m@я‡G¥@,&Mq£?»J}ãÁÂ?»&@Üi"@¦¿òÉ·@λÁÎj¿Ú—"š|©?ïòZ€T#C¿âž/`?Û¸¿ä¿ó5bB¿ç(§ß, È¿áå˜îxïAGNbcuAT20G J175822-302916?él#4§@?À¹Ýyƒ$?r¡V»œM|?m1šÉó¾#?ɺì¿JG?À}ÖzJžà?èÒ1	ږ±?¿°J£:¥?|2#ùba´?Š°[ž«?ËÕª¹IÌ?¾ûá?þü(?çïð+²Çy?²VtêñLŸ? ½*a`>Å?"V=\(‹??Ìô¸ëk?°ÐŠÊpgv?è«	LÉ¡
?œ…¾¢¿<?¤×&[Î Ï?€žúj‹'^?È5åó˜?™
õZ6a¤?å'TzovŸ?¾ªNþs?Š†äzh?†n
éuÌ?Ô
²ÓsÒW?½©ˆålUê?àô°39p?ÉT~°<ÑË?Œ	ÞW!?•d
€1t´?Ý6P§•ä6?É*%Ý# ?à
d1zBß?¸$mØ׏L?°+L»'h? XÙă²e?ÛàwJJ(?¶É—öò´??âŒO¹Ñl?©îc_Ϋ?´2'Z€R?–Ñֈ¬?ÕÚ¼¡¡ó?§Î…Ïí|AGN4FGL J1758.7-1621?ïm²Žªu@aXPÀ9œŒ…´àGÀ;qõ *­S@±€k^@*ˆŸvRm?Å ùIØf3?ÝÁæßóp%@ªò×ùP¹@	Ré¿KÚÊ?ïÓíözE?Éà+yUg¿æ™U ÃÄæ¿è	ÿþR€Ö¿ïÿÿ^ðP`?îÈË ÒÈåAGNbcuAT20G J175841-161703?æ5«B/ò®?Çn­ÁJZ?¬Íä4S‹ò?ªMö1céù?ÏõÙéôX‹?Å¥Óó¡f±?ÞV¥'}?ÑNB_Ì?ÈF;uG;?ÆS;'HUj?Ն<ßH>L?É.ÓCÁX?â¨'&
?´"Õޏ$?ÆÈ{à²C?¬žVãS±_?ЍŠ¿X'`?°?.}¼¥U?åyN>7¯U?¬Ó@[>0?½Áí~PÆu?Ÿ«r'?Ë9ÐGøßr?¥EÕÿÔ˚?à²L¨ûz?ËG¤[OÃ?µÄÐ-H?³ý]õdØ?Ù*2¢®Z
?ÉÅC½*S¢?ÐCÚç'þ?ÍW i±8?ÒÚL[ ¯?Ë}]nM?ÜáÙ|áI?̪Aƒ>I£?Ûò%+³?´Ý©rÐc"?ËASÝLÍ?±,Ëig¦?Ö~º*]̏?´ØÑŠ ?Õ,Æ&ëQG?±Cõ'Ý ?Ïj©ÐXP?°µ{aý¤?ÛåI¬''?²Ò¡ñ–€—MIXED4FGL J1759.1-4822?Ô±/QkÀ'èE™gD³À9€ƒmÞ*À;úŸ[zz@Õxèt3@µJd¨ E?¸5hÀÞ­?Â5záº÷@©]'«Ž@;;-Ržˆ?ïý› Ø<¿×ÈIe#Æ.¿áñ"ý…ý0¿ä€|â©­ä¿çåöÔÞF¿ïÿö?ŒÝÉAGNbcu3FGL J1759.1-4822PMN J1758-4820?ïá'$!"È?kØY›nZM?BÀ:Ð?•u?@}Ƨ$?i¾Í5Õ¡?jQdg+à?ïâÐ9
Z?u)fN;=î?3˜r‹Ã3û?EŸœÁT?j¼¸–(²¼?tAO‰ÿs?ïgC•Ì¨?ƒifÜ
©?n6Ó ¯ë?qã&®Õó?ŽªNÛuÖ?€ÃÓ'T?ïßñ¼½­m?NÅ&7£G?BäsÖÇðG?'•–宍8?kU&P3b›?LÝ?njÞ3?ïÕ®7¶O³?nYƒ3ª2?Tþig£®k?P'†
ª­°?oғª|è?jòîØ6ù–?ï¯ï6Y-n?`ŠžòT?I¢÷EÒÞ?ah&0ç?'jó½`û?Ž¦NJö$]?ïÓg"?KZMQ¸?{Iÿj"?|+/½_¬ñ?˜Õ@Ãý`â?‰N®Ø+a?ïªØ#ÿë?löø­˜Úx?XÁŒL¶`?Döë÷?'1łP0Ö?kB½²¿AGN4FGL J1759.1-3849?áñg>†+À«Då^³À9¼~Êá:BÀ;Ñ E…EO@³WÞcM,@pöºÜà@?À×&B	?Öæa~?¶@†®â:¸@Æïp:Ћ¿Å«.1Z¿ÜR€ vÿà©
?ƒ£Ž¿à4æÇIÖ
¿ïø]߯' ¿ì#;~†BÐAGNbcu3FGL J1759.2-3848NVSS J175926-384753?ã¦4ÿÞiz?Âm.ùß÷Ä?͕r¶Å"?ÀÇ`ÿ@´È?ÃҍÏ"†?²A a¬?ãåotÆÀ?ÊG+1Jêy?±·»&Ëà'?°ý{'&ö'?ÕrFVÚ
?Ç]Ï?Ý!XqÓy\?³ÒÝ4³lÓ?ÖY-$È®§?³[oˆ~2C?É
ôÒǯú?¬KW"Ñä?ê"Cé'»?–I®D­vI?ªß˜Ù	®ñ?†¥UJÆ^?À¿
%Œ›H?ù="ˆ0µ?×¾•.jf?Ã\Ÿ)ó»Æ?ئÒÕØí ?Ä!Ém6?Ï5/ú;p?ºÖ¨mÇٞ?Ø»ÜÙ¤ƒ?Í%Š½ò¿?Á"»¼Pí?Á=¼Ž''Û?ށÅHZH?̱otéJ?Óû6_Á[?·a؈ÓßÍ?ß(س­8?ºœ[.¾ž%?ÉÝAŒðÇ[?°Õ±éôN?ãe^ÊCc5?§3ñå"*|?½­Zba? îXxD¾?ÑÉëãà±þ?¥Ò®ÏeøMIXED4FGL J1800.1+2812¿ê''"-ý@6îð8⟝À:ôSËY/FÀ<›'pˆ(X@ î»J™VS?þðk®Œp?ȸLHß?"ˆfývI?Ñmâ=ž@ÎëØ֛X?ë,yÀ¶>¿ç›¸䆨¿çî°ýŽ`«¿ÚUã ÷€¿…QU)Ÿƒ
¿êG¶þ.n¨AGNbcuNVSS J180002+281050?ï¤!þ£?­¢5ÓÚ.Ë?Fj톷?Q	òÊpÓ?…ÞíÄ+?­˜Ò÷âU?ïšîå•4t?ˆ^?*¬3Í?X†Ú·?aœmòÜ2?†0¤XQŠ=?…qö
µp?ïSV×Û§9?'de¥4N/?X"97'"?C—¦ñiî?"Ébª²?'?ÉÙ"Q¬?˜BÚ?pVÍÓó0´?HïÄaÊ^?3ìÆ~£¾4?ŒA(Ց`s?pKKB}ç?ï/Yâýï7?°"Mgró?T°Í®BIÜ?f©â9`é?˜É¶ÂÊ??°Hü3œÙ?ïìÁ"¹W?¢5x<9²¢?cä5Q?q)ê¯"ÿ?›¡ëL¿¡@?¡B͋âÂp?î†`áäƒo?")8±Âó??c5¦Ñhý?X?c9U¢!?¦fŸø&™|?'òf2«F?îK€'.?[n^Ú
`?d»E½ƒÁ‡?[ݒ.K±?ªL¡?}õ
¨ïAGN4FGL J1800.1+7037?ëuBµÀI@=·hß½jYÀ:Ê,"ÜÁ7À<‰ep!@ ̀Pó8?ÿCxà¼mÚ?Ë+ëb<á?Ã;9&b?õàoP–@ôe¡o{ä?àœ)@ìt¿ã4>Kë¿â¼RÌU®ˆ¿ÝÜ›Ýk«¿êøU|3WE?´.FåA¸²AGNbllRX J1759.8+7037?ïvO#m‡1?´æÔ"~'?'ÀLEYÏ ?µÆr÷‹–?WÕ²Úi?nÌ`Ýb¶¡?ï¹^ÇqÕA?uíöI'*?Uy½—`ëc?W@¬²–æÅ?}ò,ÅÀDý?r
Ûàc÷?ïj=dJ¾{?†sE–üý?i™*1¤Œ@?uÑ<ló–a?
\cþä?ƒ™É
­¿?ïV6w­­ð?pÚH£l]?qaZ¿½ei?QV´0åv?àÚ\¶¢?pTdH'?ï;Ü'¼?ˆ6i™Wǖ?voP¨3š?jÌÙª†Fñ?"àõÐ[‹?"Ü"Vº—ƒ?ïFÍò¨m?†˜yÍ»#?bº›—¬¡¸?iys¹')î?"φú?(?0]ã+ ?îêã¶ü´z?HàЂ|?n´/ä–?pï½
4¨Ó?žÍ@‹½6?Ž%Ô±åÄ)?íûn'-†?.*,EБ?…\O!«j_?qSGª#?ªò,`u?ŒËYE›´ŠAGN4FGL J1800.6+7828¿ï䌳›è@=‡¤¤—À7£>d¿9À;‹Àò£öë@ò@/E@Dȍ$@?'ÃX&T?¢eÀN9H÷@(T<j@™ü)ܝO¿ÎŠ'ûG‰¿áñ<ÞC¿ãΉ/¿
l¿á؞AŸÁ¿åd]½ukè¿év"U:oAGNbll3FGL J1800.5+7827S5 1803+784?ïè‡0"ú&?UÜ7½HWØ?9ž‡'æ?.G"†•²?dUžÓ¸¢?TØ¢ZhÅ?ï«göšŒÅ?"'DÏUé?Y"‰¬¼ä?aŽ	†O.£?õp;³??ƒs<Iœ«?ï¥"ËuÎ}?ƒGË1?dì15¾é?s1ùs0:¼?|@ß"k?'¶Gš‰\?ïçÕ¶D9?Lz	@þp[?HXêlºÒE?3pAÙEÞ?b;e;ƒ?GzÁ°¼?ïÑÒ1?l[âURsg?5 GC¬%í?(|‹±Y[?u¼òƒz|S?kësÿű?ï»ë•"?¢Çðééf?j½ºqip?yß|1ø?™ßæÎäQ?¡‰ Ë]©,?ï‹.©®0?ˆË?&¼í?^زVý|?jŠ
åçÀ	?‰Y?S«bj?‡«¬{$?ïÍmtTª?g×Sy~æ?[2Ö8T?R—ÅBºœ?r‡§¿ý$'?b™Ä?h(fAGN4FGL J1801.5+4404¿ÐQ¹1J¶ï@;Þüz9'À8±5
þÆDÀ;ò×DÁ@~$žÅÓ^@uçÈѕ‰?¢m!à?±ž©Š@µ›"/Õ±@§¬áB¿Ñ<&âAþþ¿áÀî<‰K¿æ¡¸í÷­¿ã¡ a}ï¿ê+h{¿åQU]*AGNfsrq3FGL J1801.5+4403S4 1800+44?ïé`п?Uµ«AèzÏ?A$çYq?1s"¼,"Q?bUõb¿©(?Sè"SáŠé?ïã¨/ ]?ià홊¥í?@x_X¿zÈ?LyuýTi?h9ÙÇqÃ?eœ/˜r§?ïmxW¤F?Žïm˜ná?cîÂòT°?gmC›?Ý¾j<‡?‡Âb­Í˜?ïþBãKá¢?çÈݕ"?ËÇUg'>íãÙ2??'±Ù…?E¨?ùop"_˜?ïÂZ0U»Ò?{ƒ+Z*$¸?L_"?A}æÕ¿ß?{A~«0å?znø~©ð©?ï­±¾ué^?"3IÃp?Nüò*Ã?`¶æÜm?'£ÁCbß?ƒih‡|ƒX?îÀHE¥6í?œß¥¦ôõ+?m~s˙8þ?múeÏ?¢#"hY#?›ôðRDÎ?ïûº$öÑÐ?2;~¯ÔÌ?;mÛ[Õ?	 ÉֆŠ?<ßûÀb«¦?0±.;eoAGN4FGL J1801.5+2123¿ïp°ÅÏF@41GàiaÃÀ;½ôµÀ<Q )k3U@7œ9Üñ@ƤD‡?ĵ¤as¸¿§YÝÝÒj?å\=îx?ý3="šÙá¿¿—b¡y¦¤¿çí÷­K'¿å—ß_¡{:¿áÛ`C6¶¿ëOqºû?Ä}XEff'AGNbcu87GB 175915.8+212212?í֜{Ò3?­â¢Æ×?yqêmŒ?m°ÔÅ{â?¯uJ&a5?­x'Êmx´?ïjèñ?–n;¯y?~}Y&tÏY?~n\Ç.¼Ò?–ìü[õc?'ç0§òà£?îà™#cB¬?`ƒ{,ï?zÀÒú·4?z°±ùØ?<Ö0ò¼?ŒS/
Dó5?î@¢uÇ?…™ádŸÁñ?zŽãÞcY‹?`6+(?ªú"u"º^?"`¬ƒMGG?ìi¢í G?°ú$–.Íj?=d@Ž"?|e''P"¿?¹E,ª¹ð?°ƒ[¦°2¬?íšÚMz?­€'Õ?'6ä\zC,?™S}R&˜?­Ã,Uó?¦årÚïÎz?í£Fɓ'? 7õTtY@?"ßúÔV?}tód–¤?°eˆ¸ÿC?ž4¿÷½–m?é¬ßâSFÏ?£ZÿÛ?•]d蕈Æ?ƒ$Iõè0?Æ ÓÙ 3«?¢¹ÿcϒAGN4FGL J1802.6-3940?ê•R#۞ÄÀ ×d­ÿ',À7†Ã!À;/kn
#Õ@÷ZšUVI@ºÞ¿q?›0œ]¡ÏQ?Àƒä%®æ2@!+ˆ‡"ž@ –žèc¿´õ¶6ˆR¿Þž K¿åH'NI9¿å±Wü@X¿éLõ‰¾¿ì¼Ý5МeAGNfsrq3FGL J1802.6-3940PMN J1802-3940?îQK£±9b? ˜–+©eº?nô?€V1¬Ì¯w?¦¥ê@N=?›µ}&¦šÏ?ïæÓ¢îœ?³rµã–?QJÎ+ë?dí`SÇdB?œRÛÿÌ}?³6þ¬çp?ï=£"¹?'€7ŽZÍá?‡Ì#J+?Œ;h‹Ú"6?ˆË0¦ o?…,ž7›Ê7?ïêk·Å9í?Q^ëwüžž?6‡W,Sy8?.>õül?bÃ]ya!¤?Nu0ý¼#?îyãpÓ'?ŸcfUF˜?ˆ½÷î?"Tnjè'?§ù ~£?™¬ÛÅ×óÄ?îH\)ÿ?¹Ø¯üSðd?nJ[‡QûÆ?"£¯Š+Cy?©™ÔŠ­ÙÈ?¸s»mØ4?îó7|)W?˜‡..§ãR?¬ˆu	5l?ææ¯íô?'·ÔÐÎÐb?Žî$7!<V?ïÃ]瀜?o3Z6ã…?O\E£2úÀ?FŽ¥š~>`?zeƒamH?lº@sY´<AGN4FGL J1803.4-6510¿Þ %šoŽÀ3¤çÝÊKÀ:Hð3Ú"À<')H>@åWáY@;hê?ÀyYÑÇÞ?ÁÝÀåãÊ@Y%5C¯@»ž;¿É¯?Ð$¿½o·ž¿àt•žbV6¿æ~|§ñK1¿é\VbbJοâonLå¿ïÿú@ùDzAGNfsrqPKS 1758-651?ïöu_¨‡?@½³¾¶vã?3µ/&Ž¼°?+ÞÊ@á?LOê]ñÒA?:¨¹dz6?ïÌIjé>.?t¨›}gx?LOëvQð¼?TÀÐB·°g?vQMÐ6?rãSsko?鉶¥yP?u_í0.˜Ý?Z ÊšÐ¾?M·ÉLʱ?Ê}`T³É?sÜx†¡?ïu©¹2¢P?g.phaU?f–k½lu]?E/"];R?ŒïöÒ ?fªº?ïèEˆÂ©*?YU	Jð&ä?M¯Ĩ"P?HRæ	o)]?`N¶xúÌ?Q¦½éŒûk?ïe£Gî+A?'°š—9{?d¨H9NÞ?pÑ#‹?¶Ž
?7Ï¡?ïSw»šÂ±?"ߎ{<é?n´[FäŸ?qE¬¼ùâ?'Í1þS"T?'$‰Ñ•Sx?îCIÈÇ@?‡"ü,"z?'ÏŠX`ó?i	ç<Á"´?§Œ­…±F?†¥&S«AGN4FGL J1806.2+6143¿ï–OÀ»$@<ô¡7óŒTÀ:­FBÐ_À<ˆ¢üïªG@Y€Œ­M@ÒÆü©3k?Èg¨Z҉z?ÉqBãTy?õÏíé}¼@ßÿ/ögÑ?âXO'RÑ¿å9ž»'¿êi8"†<Æ¿êpBóš–ð¿î¼üJÈü¿ïÿø¨ó©°AGNbcuTXS 1805+616?ï)EQK€?»Éqçì?Šo‰!g³â?­ÒînÅöé?'#¾C~!?¬ª"¤:8?\nÉj?ˆÞôüó"g?kóUº¬Å?sñ™Pµ°?"â"p{6Y?€ì•Æ?ïrÀ²W&?‡^;¹ÿk?e½½&þ?knb"ÝêÅ?ào­<,º?…çºAq¡?ï'ÃW"Lº?e—ϐ.µm?w)æ¸ñ«?WÄh–i¨Ù?tm…'"`?^"ñür?ï£Õ±1c?…²Mx6{?l !(ß¿8?og')°˜?ÅÎ
S?ÀeªŽ'_?îàgH[?Ÿ5#Ѫþ?€-"¥u,?ˆÎ«ÿ_·š?›Ü…ì,}P?–a£¤ƒ"9?ï#(E?‰—ò´?pSŽèþ–$?p=>Q¯Ø?—†ÚӒè?†@ÊìÐ?î©í·~?ƒ­W´ðSº?'­ŸIî?v÷gãcœ?™©ö­¹?}…á8d)†AGN4FGL J1806.3+5345?ï~a½4So@<²[1~þÀ:‡Ç™kvÀ<oaÊsc@³IÁ?%@¸;Ÿé?À×Î.äð?²Î¤¾:ã¬?íü¿øÓç@y³Ž¸?!¿æÿ'æFñV¿Øò­œ…Ý$¿æf~ºC¿éQæýz"œ¿ãI‰›á¿åݖ^%ÐAGNbcu3FGL J1806.8+5346TXS 1805+537?ïúHªœ:?9qtª:?!PÒ¯}š?šŸoCÊ?Bœ,Îl˜…?4î[ªn'?ïäþ E´"?j‡ úâ5÷?=Ý߁%¨e?J
ò*țÃ?gF#£dÈÓ?e¹ø}òÆ?ï»KŒŠ+V?jKtû±
?XÆl‹Æ~ž?VU'<׉?|(ž¶5Dÿ?f
6ÀJ¤9?ïßÁÐê‹?Ký}‹z0 ?Kø=ÎZ^?0ïc—]=Ë?i@_Фå~?J/y4Øp°?ïõêá=z½?BŽ:ßZ´#?.m¥Â{? Ȁ)yó?Pfχ8x?@¹yë›Ò?ï«ó>â¥?'ì1|?P?k9¹ƒÒ?[Ñk6±o?'ûBÞyV?€øR*Oúá?ïóâ*q?{yU/ R?có¢`Ôâ^?_zZ1¢V?‹ϏO?xÈsdç6a?ïšTyݱ?nފJUh"?eŠDLð""?QõÌÙ¸?"P õ5#?lª;ýÛMAGN4FGL J1806.8+6949?탑qä!@=*½¨!óÀ8
|à%oÀ; ë)¯%ó@®MÈ_Ö@ñuù`¾?—òu"§¬?ª%û÷:@®›aöK@ÄÃb벖?ïý6Â3엿àùÛ=¨×û¿äõÔ-^'¿ãe.Í/ô¿æ].yÖ¿êo¸õs~AGNbll3FGL J1806.7+69493C 371?ï믢x?aVúœ?El

Ž??X<70)–?_'ÔÓÕH?SÏjz^ù/?ïzªå³?NxâS—Ž?lÆcÜZ­?v4ŠJð?Š#­»+èü?Š™"¥¾ßÝ?ïsª–/ñy?ŠG5Jnöô?rÕ¸Gö^û?~ÛË.pc?‰ª~OX†>?†i…'y?IÑ?k~_ñËŒ?{Pùg?a÷ÚÏêB?}^>}'î½?]>$1Dfþ?ï×Þò¥_²?nc¢æ™,"?LšÌ
2ŸÌ?Q¬ßŸ&?p}-"†s?jjò"¢±?î¾9Ž8‰×?£ÉID~?~NÒ1£Ù"?Žú⯙'‡? RŒÚbo]?¡NzGªõž?ï$7ŸKÒ?";֍æ?yÂ"KoÅ)?ƒµžÎø?•ƒ~œŠ‡?Ý"ª¨pÞ?îöÿ«
I?…ª{뾏?ubl?~ì@;I¤.?¾
¥u?wê‡K^"AGN4FGL J1806.9-8038?݀IQëÀ8öt)ˆ<À;Vm¾iÀ<±>K•)È@ á'&³ý?üþ¾œˆac?Ñcz"ÛÍ?ÆqLN÷?õ,JŸ`ƒ@ƒ»ùë¾Õ¿éÓÂõ³uä¿ïÿ½ 	c?ïü•¢i!¿Ï虚eG¿ìTտ到?ÐÑ"D¿AGNbcuPKS 1757-807?ïQ[Dý¿? ¡Ð:c«?]e·ÐøfÀ?bàQ¾«xG?›?yÀ]½?ŸÅ|vs#ä?ï¤ÝmaŠè?'a8	?YÏu®å¢?bïY	s«¥?ƒŽ¶S4?~n¬I4Rs?î<Ðæaô<?c,œ¬x¸?qtañøƒq?tÕh»¡õg?ªeY9ñØ?œÖÊáìíÊ?îÝdÖÞ?'z†\¼ °?aÌÞ^ÕVi?T¨þ"Ò°ì?¡ä«?þ+?ÓbRSQ?îŽöõ·Ÿ?¦I¿ùAÚ?g\cGÀæg?\E\]Õor?¥šÊlÜ]u?¦
ü™£h?ï­°|à?œSCÞvúP?hÉ¥rº6?ssj."·`?œ:qõI±?šÒòÅs«ã?íÆ­P',6?¡ú	c.,?rÅÛ×*Ã~?vþýǤ˜s?°ž7Âqѕ?¡é£|¹'?í-}wá?žS×/¶­Ð?pB$cöÃ@?k—/7ú8?¶jqÍàŽš?üߣ¹åAGN4FGL J1807.2+6429?ïMb ±{c@=Gb• ŽÀ:øã`'À<רª˜@ !
]¦ú*@¿»lR9?¿
…&}˜¿ŽöjÍJÃj?юÖ<b0ø@	¼‡°8?¨šák.¿ÛJÿ"	•*¿â»uÝök¿Ó[<'¦¿å0¯?ž%š¿ã}|BםAGNbll3FGL J1807.8+64277C 1807+6428?ïùÅû¿?[Qd*ZÊ6?!öùo9?;ƞé.?D§òÂL?[<ù†?ïçE˜W?mF˪Y£"?9˜nŠ<?F«Øl?	b?eš4PÁòÕ?i'흷<?ïÃfG:YÌ?g{ӝ7ê?Lïå1óÅ?;æˆÎÂk=?z®ß¨þÛ£?f¹pŽ-`Ô?ïíòÞ¦¶?Cq4!Ò$?<N"
MH?HÃ%Ä<?^ÌxçæåB?Bðv•§D?ïö«Oúi=?Q "mÙ?4°‹6ÄIS?0¾pÊÑ
?Jú{
5—?L¤îóâý®?ï¹[˜l?vX'6y?FN	Ê'_?VT΁r?€UÈrÃÁ‰?ù<ôÕbô?ïƒÇ^4$?+ä‹`•õ?TØò‰ò ?TžOx›˜?Œs
,·j¦?€ÛR9ÉPr?ïÊí.8š?`hF2?ShÀn?;¹r¬þH?v1¯gC«…?_š­ÙØ$AGN4FGL J1807.9-6412¿ïðÐm"À3ºnCªy¼À:Mð÷3©À<Ò¡"$@b,™!O@Lë]±‹ÿ?¿bVz]?³,Û§?òö`ÿõE@ÿ@±K ?ïÍ>¬ãù9¿âĬ½bÌ~¿éñ9ÉOiË¿ãRžÓ•=ê¿èó2ýƒMþ¿ïÿôÕ÷AGNfsrqPMN J1807-6413?ïꥤ®d?[ø{Ü*G?Båz6T@?9ô±ã°?` üº¨>l?W/òq"2?ïÅðøP3I?w{>êe½?Q4"wå?Zïh"O>?xºÉQ?tˆõW¾}?ïpSgäžX?‡¯6²ñ8Ð?cÌ%¬eºÌ?iT͉ê†?Žø¨•M?…éôb¦?ïd.g¾Í}?mzxnâ?edÇ
äø?D|Em¢Z?Íš'3½?l/š™i3"?ïà,ÅÇZ?e`è{¹f?P{'ܹç[?F.È^í—Ä?g•r'ÁÔ?a­"k–?ïnn³ñ?'ǏSÎ?bŽýv^?qüð>^ù?À"ï»®$?}S5â?ï«ÈESœ?ŽQÏýð
ˆ?uáŒzáÃ?|"±½î0Ì?—†Î›ÿ?‹^c9j˜?íü³Ýg¤ª?{ðEµ²M?'r©A4¯0?ifå¸"¡?«˜×j¾?Œj™ÝAGN4FGL J1807.9+4650?Ù·Ž_‡W«@:'ú'è},À;*ƒì‰*·À<Êˀœs@ 궦oÀØ?þW§6:N°?ÃÁˆ5™¿^…'Wîå?–V»ÅàÁÄ@K\YQ?ïrÿ0Í'f¿æþíþ¿Úw
"˜±<¿ÞÒÕºÝ3¿ÞJžß©žJ¿¶ìKÿC'ÙAGNbll3FGL J1808.0+4652RGB J1808+468?ïêéònê?`áyÁZÓ?;Za`?4¤Ÿjo·?buÖ/ÀÛ?[ùýÎî?ﯝto"Œ?€'—Î)‰?U¨ëÏM?X=ÂÃå*?v­ÓWÁ`?}ݶ¨íÐK?ï}4½»¦¤?v´8ÔÌ
?Y<úÅvÜ?@¿ì:NÉ?‹1:ÏMŸ?vrœ98G?\ "›?hªÞYϙ?Yo©Í˜ ˆ?:!	RX?‡/sÅ{s	?hÒ Fc?ïà_üâ6?d÷l³‡i?EÁÖÏËlW?9ºà°;ñ?j"*hQ¬ª?cp±yM^"?ïFÖþ?"Hõ,áa9?`ÇZV<"‡?m'ÁÃ?•]‡­?'¨©h)ñ&?ïôÎëØM?""]^b³j?bóM^|?Qé"?U?›o§À"S`?"*blð7ó?î˜S1ðó?‡šÀ,"Å?r²ô€I<?^Ph`é?¤$nN†-©?ˆ1ñOõAGN4FGL J1808.1-5013¿äFp6ô³ÇÀ,.ŠqÞi­À:Öé†@÷À;ûŠŸb0@fÀ'¢Ü@‰ÉºÉ•
?¾r]?¡+?¢I=`³žþ?á±+6½+@MΛE–¿èÙÞÃð/¿Ù…=jĚ¿é§1½gT"¿çÉóïT6¿ÙÙÁY|¿ïþµ}$îÍAGNfsrq3FGL J1807.8-5011PMN J1808-5011?ïöhÞÕ|¸?Dž|÷É?*Ï÷ähéH?á¨T/·?O¨†òëcb?Bh'àÄ?ï哞
  ?qØ.«?1kç¯ÿ?;"íÄ?h>å-jÁ?p×¼•?ïlÔm)Ï?"Ï:
Höl?e¶e¡×@?fÌ=¤‡?]`ýGž7?ƒo*ÖP'Ç?ïÁªúêíI?YEm¤F'w??.³º›C8?$¨ÀYï?}7—mݺ™?XB°²ò|{?ïëWÌgµ?ZîéD	>Í?=[#½™©,?2ž"Üã)!?`üÏ:çÍ?X½Þr®Ð?ï¬Z݊ú?'›€ñÏ]?H0ùŽ¡?Yž³êÄ<?ƒfC&i?'éƒ?NÅA?îèÏR@È%?'\
Í u:?u³šuYlÝ?w
%PÕÜ?y/"-)?!Ži;2?ïFA´Åö?y§âž¤}?[8‹ñ'-?J/k8I-´?•"@­ImÀ?xtwìAGN4FGL J1808.2+3500?×Ëãî§h@7uø>ŸÀ:&ÀMb‰bÀ<=JYPÔ@,'úÅÙi@ÿ:Þ"_¦?»7ðÝ"Zs?°_y[X?ó;ëh™@	âæk"?ÄZ÷ÝǛà¿äIÜݼY¿ä&»‹[é5¿áHí¯›d¿ëª¥Gá@?—Ÿ÷y7AGNbllMG2 J180813+3501?ïÜöÎÜz?`Ê]'jñ?S¥_@V`?CÊ´È+?i6ÈŸÈ?[˜Ë½R^?ïÐÎ]+æI?u#×oÅå?Lr©ŸÕà?XY×$P)¬?t
|ü~?p=…ÌÿÞ?ïqŠô\«?ŠnºMZÿ?r•ü!=XK?|Us®/I5?ŠRDÍ7Ìb?…HПq÷?ï'& ƒ¶·?ey9«áƒ?l©ÞYÀÒJ?H‰•XfŒû?ˆLYx3œ?côóP©ð?ï³å"ç$´?rî"‡U¥?gÿ2¸×|õ?YÚÏÅÖ³ˆ?z
œÄ…?m¥è^ž?ïsƒÚÝv?‰†Å<ÆÁ?bWȹû¸j?m$–ÔŸi?Ž‰IŽk–?…EŸ·äßó?ïaÖ+<¼?'ÇéI?{½nz">?€äV·ŠÛè?–Di¤Nøb?ŽòÚ=þ²0?îtèPЖË?ƒâ	S÷ˆ?†ÕàgvkH?k§º3	4?¢üÔÍuŠ?'gœ‹'OßAGN4FGL J1808.8+2419?êh	Y"–@3¼c¾ì9zÀ:Ïì""9À<XÕï‹=¶@ D›—ËŽ3@ð+[Î\ð?"J_Ÿ¢È?(BŒ;À?œ¼bØxÂ@1øûÔÍ!?ᅥ",˜¿ë…ë1;â.¿ÙÍî \+z¿è/V•8¿Ä FÜÞ<â¿Ý‰/žÔAGNbcu1RXS J180847.3+241923?ïM…¼9y?\ªç$û?Y^ø.ŠŒø?I>x›*"?"¹XþS?‰?úޒxç=?ï~î+°÷ž?‹eáØ£?aOñJÖ¡?hˆ´ÌD.?‹ðxËN2?ˆ}ù†è\¸?îì:gÉ_?Ž}ú@sC·?cNzX)?]?Ìôqû? *$—v?üô´|±È?ïw	KO¬?o²Xò¨[+?L¬floæª?8Èù=?9sjæÚ?oš="1B—?«W ë? ?å1^·?mÛTˆ1?bÖbým*?¥‡˜)ð?Ÿvº´`n?îõj¯~ç? ù@ŒüÁ÷?e­Û§§k?r¡´ŸŸ7&?ž»üõþW0? <¡ôk~'?íRû@\>? Ún½KE;?rq]¢áه?m²Ž	Nýy?´A$ª9? s> ƒˆ?î ¾¤k?'+Q'êôŽ?fä&ƒ>
?[š+…=ç?¬h½ûðô?'+RM±ŒöAGN4FGL J1808.8+3522?çªÛWÌg@7s²$ªÚ4À:ß\×qk}À<u¯§"Y@³ò ™R¢@EĚÏ#¿?щĄ©Èf?ÚPÓ!z¤@w|7‰?òI"Ž³°¿Àgّ×-?Ѩ¡ÿïŽï¿àx^졬¿à²öañŒ ¿è»ã?ÕÙ¿ïøbý¦3†AGNbll3FGL J1809.0+35172MASX J18084968+3520426?ê`ðO€=J?É¥ìýށo?¶¹Æ§…Ï?Ũüvð?¶>¶ÝÂÖc?¸ ÓÂÜÊK?æ_ŽÞ§«?ÈpAsÒy?Ë'ëè'4?ÆS`i)?¶³±;lÀ?­‡À·ÂXè?í1jEC+?¡gd:òW? {ìe''®?•ÝòJ?&?¬rÌúd͚?˜¼Á¡Qr.?áÌ[[N
?¢ÞÃ_ß»F?ÐÓVd÷¸?¢KêÚÁç?ȖëåýÜu? ¤¢$AM´?æKÝ!{?Éñ-ۖ¥Z?Äé0ÈAD:?Å;N×öÃä?ÁêÃÅ^Ñ?ºiоžá­?Ûþ.g$/?Ï+b¢j+K?ÚÁå\Tƒ?ÏàÛ_ë*¹?ÂØyšß?·s»ëQh?ëSÃyÅql?¨aÃþþ?¨]kr°E?š>®¢¦nÐ?¹3cúÑAü?¢ò+uŽÑ?ÓG¤"£\Ö?¦D=:«Ê	?×(àë	?³a݊1Z?Õµ3Í{¸!?±"#Æw¬MIXED4FGL J1809.3+2042¿ï˜ë7µ¾@2Ao!öÊÍÀ:>Ï#¿!éÀ<VÇM1;@†Ò£¦bÖ@§—£öî?º£ÅA"¿w8uKï?¾]‹¡^_@Q
9òÑ?ï\6f¿½{B*8¿àŠUú˜{¿ã®bHŸ¿Ömt¢"?¿âG àö$ŠAGNbll3FGL J1809.4+2040RX J1809.3+2041?ï%¼‹=Ï?¢¾ÉÇè?"?kj·À^r?q¿DZKü?—ÛŽ+ã?¡-Ü:¶±Ä?ÿW8¡?‹3=ÃO¸‰?YFI±Àÿÿ?\‰¢HôIk?‡k¶ä+ƒÔ?‰®¼ïÉ¡Ö?ï6•¬Ù¨?"îî,:gý?l©Éç;?kQUiˆ>±?•¬µS#?ƒ'¿Ç¶¤v?辶¾+…?uy]¢ê—?rŠ](q.?TÉè'"pî?˜èC'Hi?t!±—ój[?î3Gñcãˆ?¢wÒÅ@X¹?wœÕq™?w¯_wŽ?¨m™°q ¢? ¡wDÁ6R?ï'‹æÜ ?˜<¨õ#¥n?gœz'þ¦§?pl]âæj?œ.ý*?—bbûƒ×?î`
u¼ù?")åV±g—?wôY7b›?oü\Ì"œ§?§™÷ªŸ?'¥ÌF®ÔÙ?ífUFOçì?zùåÜ?‰2ŽŠ¼v?s þGÎ?±§
YCŽ?_¿!KPÍAGN4FGL J1809.7+2910?æñ·ëòµr@5EV:Ÿ8?À9ƒ-±éòxÀ;í.I¼â@ꊁù"×?ü3=D.-:?µ'‹>s>w?¹Æ]qö•@Xå>³™ö@YmÇXÅ?ïàCß銿å×Ù`.¿ÓcY%¯g¿×#¡šÄçÑ¿áa'·'I¿á€0q·ÓAAGNbll3FGL J1809.7+2909MG2 J180948+2910?ïøfüR:?9 'ˆ'¡?)+ž·_x?Ô}È­OO?I«|™þÚ?6KŒÜÕ:?ïØÄbZ?t9î'Ǭ?N
!³a?^øÍm›ä?o›¤[øwî?nïâ]N+?﬚Çô?ttNÏMˆ?^¤VÉ&ÛO?dCYObm?%Žs
¬?q-F–†¤}?ïڎαÌ?r9¦k™i?lžÛ¦C?GÓVÃ@2?›PÒ°…|(?q'¾œD)?ïóZZ"v?G0?64¹ÐG!^?(·.ý6³`?S¾ð¨Ÿs?D§ë4íw?ïvÍõì&?Ž	ù_Cˆ?f#—P~?p'Y•¿?ŒË¹Ð'j†?‰Â¶éù'Ú?ï××þë>?ÝýmqÒ?h¢',Ž›?pAZͲÏ?‰áemê•?y"áåaeð?íËN47âg?ŸQgÇQ?}!6(ÿë?aéêû›A?¯¦öPF?ŒÖŽ7RâAGN4FGL J1810.7+5335?ï×l™Âo@;i_JsÀ:[Þây|À<'d}Xs@¸ŸJ;?þ¸\'·ÕÅ?ÂÜýŸ?º>—ãåî?ùž˜5@ "ô>?ëf?úìÆ¿æ‹vÁ¿ã±MëE]Ø¿Ñ¥øã?ì¿ãÃ?»òn¿áAÝ¥¸AGNbll3FGL J1810.7+53352MASS J18103800+5335016?ïâ!Œ†zr?hT"HÓH´?JuPïŠ?G¯‰gÓKš?g]VV}­?cð¬ÔQ?爫ٳ6?}2)"q?_ÇÛ9Œ¿?c"Ðٍ)¾?¤Ž&‹:t?v‹o¬­"ñ?ïƒ[Æáb?v]+4MBá?aÎéS^€x?V°¢ †Q?ŠÄ®»×Áy?u?ff¡(?ïŽÃÊ(?tkcÌfI-?"퐡)Y5?`­¿!Ý°(?"_2¹'h?q\º…•]L?ïÓkä÷Þ@?gŠ6rSi¿?V½™ôHiä?K훇"?pš§'ûj?cË+†Ç?ï'õ­Ÿ?"¯zg¶XÓ?s"²ÜÚ?x×ÈÔÛ?˜‹_*n#Û?Õ<•¯°?ï¯U÷?'Þ+ôïcw?m%—‡"K?bfŸ‰üÐ?˜…bQš+¯?€Çï¤Z ?íb²ȝà?D&4B?›>§^þç?€E®
?¬5‹ÂµTˆ?‰ž·)'7ºAGN4FGL J1811.0+1608?åËóW"Ö*@0ٜ¾èÀ:UáE)Õ¼À<7tm&S@ •R&é?ÿaýKÙÆ?ÄTPåÔÝ?À¾õHÁå¾?üŠ=Ü¡@
ÐÏ֗{Ý?é?÷!	:¿ékÞuk¼ç¿Ý¡ ñ§£¿ÐúBœÜ=¿çÎ8§ç:6¿å´ ÓʘAGNbll3FGL J1810.8+160987GB 180835.5+160714?ïîZf±m~?UÅÍT‰%¢?5¥Ôxñ?)/|Š'‡?]á½1ÍÁ?TfÍe`Cm?ï×Èþ®h«?t×£Ð2<¨?F·³wɊ­?Q¬Ý3kÉ?qDŠ7É+?qŽVY"çÿ?ï˜ôм)?{V/Ý¡Yú?VÔ(ýyB?\pcòÆ"?†èIÈ#"d?zúʇàK?ï"É:=Šò?dALJ¹;:?\m°üƒK?>ênÏ?‹?û@ô)?c~'(Ç?ïߍ-ÇÛÄ?e±ð\ÜÀY?G§°y9Î??vٓ	uØ?j«(H,ÄK?cíX¹ü¤Ð?ïÑeýy­?DJ¶UR?Xfyâ¿/Z?jÁ°b«•H?‰~×M8ªÝ?‹'ój;?cú?+=ˆ†'Ë?b$G;§ç?a»»ìûww?š‡#ҁµ?Ž€ÅÜDnW?îŸõe6Y?ƒ¦vŸ6?rå2Mrã?\Ó4î
Ø?£¤f"/?'u͗¥AGN4FGL J1811.2-2759¿ìT˜ÝÿF"À£D^Ô¡­À9ðb¿¤À;¦Ù>Ëê@ r%|ç1R@
òœj.r?ÁÅ[¿Cw?£P»¯C$?æòûE•‹@–šÆÀCR?ïI¤^ïz¿å¸ýÿÚ¿åìŸÀÐU¿Òõ¦n"2¿ä›…AÚ¿Û``="(AGNbcuNVSS J181120-275946?ì»H¸M?®/QÚƾ?gbµÜ5?'?VíÁ2?¿?:ñ™?®ž"	ñc?æ…3]Fú]?½$<J^?sð.­½?w<Œ	M…"?ҥ؋`µ'?¼à£?$?ë´©é%¦‹?¦ã=Z1,{?"îmu=2ª?y«ž+]&¦?¿¼ãcÓ?¥Ý"‹¶Ù¦?ë‹8ÀxÅ?'ž½A×E?€Ë6Ò~'\?`<ÓíÀÊ?ÀÆjŒT¦d?'=èÖ®?çß~ñÄö?º#¶ˆ×?z'ß(|}?lìÃÃÔ͘?ϯËxüc?¹í½aŽª?Ú-¹p=n?Áþb;^zà?vî¹9ÿ¡}?','åxQ?â»EՑe?ÁñõÏ9Ê?äÏo³…í¯?µb,ÕQÿÈ?–Õ8.¯:Í?†g2Chh?ÔóͶºV?´Ï€%<@?ä‡óe¬›ï?§.4Ÿ@Ž?—'Ä(²}v?¹«.*Ùr?ÕvüòÀŠ?§)'ma•7MIXED4FGL J1811.3+0340?ï3ªXrv¯@%4¢v·íBÀ9-Ôx'¸ÕÀ;®n@O{h@ßqÎ#Žû?û±ëºÎ‡?±zƒ(éÙ"?¹£Íúõ)7@2‰¥/ÏÑ@ ý+¿ïÿýFKê?ïÿàU?Íu¿Ô¼Q?Û0¿×a!§¼r¿ß
®ñð¿Ýî–áƒh*AGNbll3FGL J1811.2+0340NVSS J181118+034113?ïôÛ´œ)l?QK!à|6o?+E"¨kÈ·?+©°îþ?RßåÜOæ	?PLêéVo?ï¥-=Ë~?‹'O†§^?UiK¤•_q?_[æÆI+<?"‡;{´µ?ŠwGñA‡p?îëSñÜ?"~n
˜¶û?z«ec7è?'u论q
?›ó¼>£îv?'&ü_.?ïü;q½?x
™åÉ?p³ÑŠíöe?Q¦{;¡÷û?›""*c?uÉøõS›?ïìý½87Ý?cklD×·k?6‹Îß?5€'=a?`0ÈãÉ¿'?b5V¤«‰D?ï2qx@ü?ž"i@?g·Û?
?vüeÉ4ö-?–Ñ(MT±?Y8Ÿf‰¸?X74Ü?—ŸJÁ@èÙ?{µFâRF$?)PæŠS¥?¢Ïћàé?•-À‹(›2?î|Nã›y?	šŽoÇ?}Ë$ç}ï?gˆ½*yÅy?ªþÚJ•£¶?Ž%çËIͦAGN4FGL J1812.9+4249?àyàN3ê"@8ÅAt>–>À:–´ -œñÀ<g&••þÚ@¶-÷ `@s¤<ŠÊÊ?Âù©d<ën?£ªËñº?ß)í9SÞ¤@q‰¢¬=?ŒUe­È"¿çÏ d#–¿ç(9À.e¿çê	*v¿äµ`iÍ#4¿ïÿäâBTäAGNbcuNVSS J181308+424853?ïʧX]?ptÅÙ¤ZÃ?Uór‡•¸Ê?Ml"Q'¡è?u/–Ož?neõÛz¡?ïÈÿ"0ŠH?téàæ؏??NºZúû?T—È	¡Åß?w¨ñ÷¹Àm?q;ƒŸ>l ?ïpb·ú˜?vxþŽ¨?f¢ÇA.?`?ý2ӌd?Ž>ÊÓéÅ®?s'¼0½û?ï«i-s´5?^
޻ĵ$?cÂTžFãM?D%¾³Ù%ä?€5sòá?Zo•{¿J?ï…Ê9R:?hsùt?hã¦@¬Þ?b†p'ÿ<‡?ˆ€cå"U?
6YÂ4â?ï[Ï9—?ŽB_
;-Ò?a×u÷@ÒM?h;®å?'b—aÌqà?Œ\JW ª?îÇ6[w?ŒI}]´ø+?wÏúßó°½?l7¹±•Û? 'šórL?‰	û}û‰?ïÑ:©6?|9uçí f?}¡öyâ?d掵}	?˜@´šÑÌ?xbeÊ8·AGN4FGL J1813.5+3144¿àø¶á7Ò@5`RÚšÀ93®üm¾À;Êù²Þäý@çƒzú@E"FK=ì?¯‰ðÚB[?¢èׁÜ9?ôÌF嗞î@
KH¨»J™?ïñè°X"¿åT}e†l–¿Ýs>#§$¿äloàŋ¿à—¦°'«¿åbf'P¢AGNbll3FGL J1813.6+3143B2 1811+31?ïì;jÂÊ?RUz–V;Ÿ?6FWh³`?$د3m?`ûʐ+a¦?Q&q7Æ?ïÓAA؁P?sÞ]<ÌÝ?N4­Sr¢´?UV‹ž¢vœ?r˜É{»¸?o尜^%À?ïtÓÕ2Tš?…¸‹'¾à°?m=ŸËrfÈ?u´&àñð?‹{¢±Çíþ?'u,î>?ï#ÛÉ·;
?r°Gà˜·?p,+†ÞWl?LIÖÙ?—y{ç¸þ'?qŌ¡Äwr?ïÖvMå?j'Qy)—•?Dø7+{?8à" ò—ê?rS½þdÈ?i.]§û-?"ñ$N?‹(h҂?_b·Më5?i!'m£¹?Šè UÙýí?‡±–ãCÍ?ï1dËux—?Ž£h
¼'¹?r–½pö"?x^+[,ß?•-á_Œõ ?‹xvÅji?íœÿXvtã?'ë+æ{Æ?‡^<õtxÝ?jÏdRJ/»?°,=/ÖP?úH
6 AGN4FGL J1813.6+0614¿î[bIKM†@&xžÛø¹»À9…È•/§À;Û$
¡C²@kىô‹?ýñ ¦ÔÀ?¶•ÄÞýã?ÅyÞonM@¡ÃA2Ð7@	H€ô1?¾¿·ë˜iî±#?ƘŠ:N¿Ô>ðÁ¿ݏO(\?œ¿ä}Ëùï¿çK`6÷cAGNbll3FGL J1813.6+0614TXS 1811+062?ïƝ^þ?p!;Zu?kÔù"f?dæ]ۓB?mŽ·€ê‰?aš°¾ûÞ?ï
‰™¤ßÑ?¢MY}‰h€?v¶àüØvÛ?{µˆ0eK}?™…¦¦%? '˜–ÒNs?ï[ãÔXåÓ?†'Lîý˜?z}Þ!eÚÀ?~˜[I³mw?‹È̵ù?Ӕ¤S½0?ìKw¼?ŠØé•ÏB?ÈšÃM7º?g¨ÈÓÇQ‰?´XD«2±?‡ë¯Óý¢?ïji`ŸZ¬?‹g[-XÐ?">wóÎ6¹?€ùóî(õ?'/èz¦-?{ÖS}8a‡?í']°èÉ5?±ÏOT™7ß?=dTü!?–Ó`~‰·"?°o
ýÐ?¯]¹ ss?î®èA-­ô?•ËÕÂCû»?i	c>j?±zqì¤?™¹îw>?Œ¤'C°'?é*Hs¿Èá? j?›Ã·È?¡¦>e?_ˆ¸3*T?Çô«b}?ŸØU龑AGN4FGL J1814.0+3828¿î•;àÆ@7dÝDUÀ;l$ˆþÀ<¤$u*Nˆ@Ùܪ»U@!€[2•?Ãé•Zo¸?€ËŠ#ý,³?ÁQ׎â@…DM÷?ï˗C¿äª¶ÂŸLa¿èo,s%'Š¿×j,#tyO¿Þž^då1ó¿ë/…>BÛÈAGNbll2MASS J18140339+3828107?ïÀltÉ?†>'¥>ò?M£nѲn"?LçQ¾?|'XpZ?…š}·1?ïËøŒ¡Â?rD£Çh¬?Hç_
Z¸¢?RãЈ¼Ò?wUó'‹?oy
ƒí¯ù?ï{O†¥÷?~Dt/œ	¿?\ϗV]Z?U(˜:ùïþ?~¹.åd¬?}QÚ:ŽS?ïÇ,Ãh±+?UéhÞé?Kýh¨`Ò?0V-åü8O?xéñQLÆ?TìhܪëÇ?ï·@AS\?s©Þ¡§æ?R;hH,Ü?Bxïsl¶¾?ÑqÔ
³?r%‹K–`?ïyïÅ 2»?‹ÎÅíNÅ?UKº`¾?`ÖYååÒ¡?ŽÚ—C[§ú?Šp%{ñ…?ï/¡5ù?ˆºñäüqë?g!m̀Þw?[ÙÒ°mÆÚ?œzJ6%?‡è~{}q<?ïE= ¹7]?v¤"<j?gAyû…¦?SÇLõ™ý?"p)ôö*¢?uÙ¾~AGN4FGL J1814.2+4114?ê£C{w<@8 9GIj­À;²_c<æÀ<…"f+®@ßÁ_±@@h–<"?ÍøU¼ ì?¿ó¬-AØ?ð+uϏö@Wâko°?îQ6ßD—¿ÝÔäžO¶Í¿è08­¿è´" [Tº¿ä2ÙaÒ£¿ïÿð`OËðAGNfsrqB3 1812+412?ïÉùë‹KE?pËE—ŸÜ?QbS"~?FLGÞX	?vªiÙä¤?n̪չó?ï°¨!>-?|›¡:[žG?[_ÃIÂG?aƒ$ÌõÒ?€jLqä?vʯ'?ïoDDí3¹?{}†fגˆ?eëFˆ8Í?dq2hü"?Ž´%=s?wÄ̝Yñÿ?ï™#Ý!P)?b—Æ5þò?d¶q£–F?E_,¤Í¿?"‰l±¼?a…Ýs'ÞÁ?ï')32ºñ?€Ì["D°?]ôêI¿/?S#†Ú/¤ô?‡÷Þò?,º&Ž«p?ï+@6À 2?•²D6FÖ?k_B ƒ¡?v;v{ï$?—,Õfz?'újS€½?îÏ6åLþê?Š—	ßaUÚ?ugÆÄ
KC?n°Kuÿ? _˜Ó]ù?‡¤LRæm?îÀؤé¦D?f~0«›?{ŒìéÌ?f³¬ðWy5? 'DZnÄ?€¤Ë>ÀÏ¥AGN4FGL J1814.4+2953?î?—Ï·ZA@4¹à`þHÀ:œÁr%·À<1ýKÙÆ@¹‹cÅ@EI@»²?Ņa(c÷K?³ÄÓÚGó?ìö®G¦‡¿@
è§á6¼¿èIžŽ‹t¿á< B¿çÄä þé¿æô,Ý®œ`¿äª$+X¿ïÿ6a;aAGNfsrqB2 1811+29?ïõՄ¬L¥?Cãd'Ž
?-oN1h?±µå|C?P§áÊ;Ì?B=oQ¹:?ïß •r~´?oœÂðâJ?BOeËtæI?LFYÞÛ¹%?kˑ
,?j!G?[û?ﬡÇ÷Œ$?p ᘪ?^‹	È#šb?cìœRË?,Ç¿¤?iZÛ¬XJ?ïƳhÖ5à?VHcÏ8ß?JÅÜ÷žd?0œ?Á›`ž?yMô_þå?Ur"‹!R&?ïïá/Átæ?Péÿ'¬?5¤ìgB?)¯Ø/zß?ZÔeÌÓLØ?O	üý^Vè?ïžï"æ6ß?ƒÐ/òÒÁ?TË¢¯²ª¡?a°¬³
Y¤?…ªªmdM?¼g®K?ïWÌ|<^?'¢´Ôdš?lTÍíH?L?lrÞÀ¯þ?'',º^M?Ñt'u_?ïShýfêè?wßͅ"d?cÝÚÆr†(?Q&ú]?"$öÏ??vû–<®ŽAGN4FGL J1815.2-2715¿‡¤šXÐ3†À_óÂîÀ9f}å,õÀ;7sx @=ϕÿÜ@®ï¼»Ý'?Ã_À‡'?Äÿ{á!îg@±ÕÝ톁@~žHªé£?ـR`J¦?íØRÂD³Ž¿åþ‹÷§q¿âÊ¡yaë­¿ç&r@T"¿ìÔ(᠙hAGNbcuNVSS J181510-271304?ê썺hF:?´Ç-"å_(?'HÀ 1œÝ?‰MYoÌ°?±­:?³Þ}º-u?ׄ>Ž0.ò?ϝEºc-?²©ÜᙗÔ?±'ÂJiù?á襦÷?Â--W–?åU4NUn?°¸fcÏAÎ?¤%p¯˜óý?'ö÷¼¼=Æ?ÒÐéNZ"ƒ?¯G"½1^?Û\v3Ê#?¢Âå…dà(?ÄJx+,K?œ‰[ÆÀ½L?Ú~MµŒá?¡ÌGi%R?âä՛í ?ÁzÜÙÏ¡?°äfñäyá?¤cQ	è?×½˜3Šh?Á¸›^ã?ÅÓo
FLb?À¢$L?¹rÑhCßt?·ZÄG/Mý?ç\ʸg™?¢Gšë¡?×Êu¼ge?±ÂT¬Ë<¹?²óg,"E?žÅ…À$Æÿ?á¼X<pã\?²A@ù˜¨p?Çuû=è1Ç?ŸÌ²ŠQ3?Ï}D·™6?©ý3՗&?âC0žA?©ôg°éAxMIXED4FGL J1816.9-4942?ÙZã°ÿ£À.U¾'bEÀ9¡ÑÒÆÀ;ðH±I¹‡@mÇ՗ Ã@ôÉBԐæ?¶Í¬½?Æ®÷ϯÖ@Ðì1"@\ÁÂ,µÁ?ïøè^£¤_¿ã´¼j~ùÛ¿âqÚ}ºjõ¿çƒüÿšs¿éâ@!-L>¿äÔê"H)dAGNfsrq3FGL J1816.9-4944PMN J1816-4943?ïÙ͟8G£?cG>Žù0?_€ƒàÖ?XIs2ZŠ?frRƲ9?V‰lkŒ?ï薫ÂTè?qËÞ¾F?4¾áìÇ7?BÜk¹m€?dÑx ¹?páØc`"?ïnÎt—¬…?"m½0l@Z?zÇf¥Oq?~%ûw
2X?†è¯'w?z¤|¼QÊ?ï¥Ç¥Ï¦?]ªoõšB)?[ªŒ˜7m?=²|‡²ü,?ƒÖ[¡?ZÒ­·]Ï¿?︱o×±á?rBÇ´äÀ‹?qt~¤Ô[?jWäáH1V?r2Éò£N?ao!?ﳩblD?ˆ/'¦[J´?V']5gL?oo-`¡A?€R5<,íþ?…TÝÅpø?î÷¼ÖøR?'mD5•âK?Œë)ÃÚ¼?ŠRt'^¿?''êëÖ.I?…åÅ­xè'?ï¶m²,…?}§×ÚýÔ
?rô2ÿ˝?ZLá'?›%‰C¹}?z¡5w4¯ªAGN4FGL J1818.6+0903?înt´ È;@&¸÷QÕÀ9S€éŸkkÀ;¨J¶Ýw@÷—´&¹@#z›§Ó?µ8ð6‰T?ò	½n
@
Jè[žŒ@(2Oˆ~i?ÔÒ«3=¿ÜºÂÇ;=¿å?çÁŲ§¿å{C؜䨿èeçPÑÑ¿ïÿ5Õ¤â£AGNfsrq3FGL J1818.6+0903MG1 J181841+0903?ïÑß*iØX?z$Æê"Þ¨?[At
ËÊ?YPäoç…?p@
®ã±?vªAómˆ?ïÐQjð}›?ߏû;Ç@?H8tç}'Ž?T²ÔƒCy¤?tÐ;ڈ4Š?}[ùKî†?ï`ÞÆۂ?…žÇ,¯€?vR@h¹?yüªþh?ŒÓÄSO´þ?€K}¶úô?ï©.•"§?a}ßÖÌa?W©îÔ)j?9Â{ÅP?'Å6pùi?`ϵ'~Û?ï¼ýcy[?sß}2î…?dñÃ|åµ?`|­Ië?wlÛ×só?nÖ$Om¹?ï‹DN0$?Ž	õ_-±?\ë«Á"U?nuOðP³?‰'wUàq?‹6Ìj³Di?îë ŸÝ«l?'(Z"^]©?…ÌÁG6Ì?"ÉWº`•j?—µ‹d8?‰2"Ã͕b?ï"g+Û
?€'§æM!R?mйÀOkÆ?Tž¡M"?—ùN£'û?{Öð§wAGN4FGL J1819.1+2133?ÚM\ù™ù*@0~ýX…ÓÀ:P-zŒŽÀ<L|tÅ¥@í	Yp	@tw·?ÀɤyF'á?ŒkÕÄ ¶ø?ϵwß?øüyzë-¶?òÉâ¿è,YÅn3º¿çe`¬é¿ÊU?øh†ý¿Úð®=ës¿ê¨U¿O5ÈAGNbll3FGL J1819.1+2134MG2 J181902+2132?ï¡)<S1D?v¥²m¯<º?W"­pû?Eï¤]Úá?"žOV`|?uŸ=)¤'?îñ°£î©Ž?¤y±¾ü?rù;W|c2?€A±ýê?œ³'ãp?¢üè<WP?ï.dÔç…?'ߘ‡òça?kõÝ|Da•?_ÖkFËó?–´©Ó>$*?ÉM@™…õ?îI¼7íò?ŽÝÀEn	?…Ê
7¬ã¥?f·ˆ÷VÙ?¥ûÁ°Mµ÷?â
¯ø¢?îúْ$|®?'­ŸŒ­	ÿ?l¡"½qŸ?]·rmfÒö?%"ü?ÝT¹¨ž=?íS¸&!§Æ?´<RÕÑ3?"²ä°3[?54°¯âf?²Ëâ>"‰f?²ûÖÏv9?îPv'Ü?"qëMíþß?xN›Ø±Ý?p"Djé
?§ü.Ç
7‰?';O*mc?ëRI³þÔ?™Ü¯ëUÿ?ž›:.Ë?†§¡ê×ìê?½Æã¿,¦&?˜ŒÐ©lñAGN4FGL J1820.3+3624?ÞÖRè/SÖ@5Þzt:À:"Y~À<ƒÎod;ê@ èíˇ'?ü5ˆ]13?ÂêÄ.˜š?§%E<}½N?轶ÿÛíÒ@½rã¢QN?ïêÒa6PÊ¿éV!IÑ°¿áãп "`¿Ê"~èx~¿ÑÐrß­*¿ßlg1gAGNbll3FGL J1820.3+3625NVSS J182021+362343?ï‹FHþee?…" jìxˆ?N'î!a??dž6]Ì?‹Lô¯§¾o?…	¦AÔ¨è?ïÀØÁ]éü?x•Ž*?M+ª˜¯š?Suäaן?{î*
oR<?uáﲡ›¥?ï4DzSR?Š¸són?\2ŽàêyN?T´=ܤ?—£àÈÁË?‰çCE¤úÌ?ïqC«Ã?j2¯ývŸW?\Ù!üÍn$??0{yK—?	øw+¢Ê?i勞"ý?ï…¶ýqt?""ÈŽA?`š"Ř¡/?RÞr,"iþ?š¼¾Û¼b?""@eÖ?ïf?ø="ß?'¢?öî'?[®¤:(è#?ipmK>	)?'}¶bÓ?–šˆB^h?îž~Êz&?Ÿ˜qWYy?ew²Û1Y?Z6½ow]?­NœãS‹"?žü£Ú.B?îLÐ@}QB?ˆ8àÖ ßT?ti®‰.¬*?a3ÿß½K?¨¥Æ&)/Z?ˆ!+NéAGN4FGL J1821.6+6819¿Ýâ]xAÄ@;Ìú¬Ùè>À9<f0¶1À<"øR@{ó&þœ~@—AЄè?«'ÈûîÃ?ªâðz¦å?÷ÀW xF@9Ê&)?ª
‹ýáB¿çö!ãÕ}¿çÛÓ/½\í¿ècúÿæ¿ëÑT†jí¿ïó'^±ŽAGNbcu7C 1822+6816?ïôp¿¨&?H°à¤Sñ#?5€*Æ@?%w¹…\$"?QÛ¢7(ßh?EÜó.+FÙ?ïÞgyl¹?n'u¥Ì•^?C"™)7?O£#õg<?l·`"æi½?hå3]É4?ï¦,ÏcLx?}ª™ZÕD³?`m®
ïj?d"¹K^ÏÎ?'Y`¤q˜*?zô{¯§6¶?ïïŽT…Ø?B\~#……?H0Ã9Aâ"?1KOÞCe?TÊõŽbZõ?:üÍ¿ü?u?ïé!äx²f?a:g'×'?@ï!QYœþ?5Øj'´X?b¢ScÁ¦Â?^è,PÍAL?ï¢!ÔwLN?†R^ñe?TÜ/âäð¿?d5­ó®?"Ü÷VPS?"JªOt´?ïh6}?›Ì?"Î3r}?e·fqã™?fao–ÆÂ{?BC‡ÄN?'ÑöwT ?ïÌ@½àJÙ?f»ée·ÒX?eâ.8ñ?WÏjŒAÑ?mÝ/]Õ?_¶þÉe	AGN4FGL J1822.0+1600?ïz't}'@+0Ãóà7
À9úmû†¼À;ä$>úè@‹hÓ©@2¼›&b?ßàŽ¾?ÁjýyèÏ7?ø¥=§*{Õ@(",J
æ¿É]q¾‰¿æ@³^'°Â¿åJ*Æ}'s¿ìÿGþò8í¿ÑfKÄ#°ß¿ïï©:÷LÓAGNbcuOU 134?ï!®cÞªM?"Gë뺽o?eFîâXr°?b¨î—"?™!U°Î£î?'C*ù³?ï3b•ÌZŒ?žKõq½¤¿?m
ÀÇ´¹?r!ÃùÜQ?•òU%)ò?›Ÿ)ì?íòøœ£((?˜õ7=óš[?‰ù䟏?"ú?[;ŽA?ªR5€51 ?"Ÿ¦#×þ?ïtŠk~S?wÉâì'ú?k¯¨~Ù?SðmZ0V?˜ÝÎs»Ä?uʗZP‹º?íh¸»`?«¨8ÛÎ#?ƒ‰ž'´'?€w¥)Ïð?²Ib:tÕ?©HhØR?îºet¬ƒ?°0ò_Z8?'¼tªiÓ?íõÿZš?ª5<zi.–?¬Ðp¡}¿?ê±bSÒ¤?©'⪶u¾?¦!Šôx(?—RgÂ69Ü?¿fܜ½TN?¤'z¾á?ípBWéK?"G–sr´?ƒ¿–Y!r)?u{\y?²úsï¨ÿ?'º>"`*ÕAGN4FGL J1823.3-3720¿Â««KëmÀ%íîÇÉXÀ:Î/OxäÀ<‹Fí$[)@@nå»Ü@Ô@C¼î2?Ôæ|+õ|?ïÿø]Ê5™@Ç%Þ¶Ú@›ëƒq9(?ïà7]d_%?èïÕ¿èÀc'†W¿ïþ.~Ãq?ïYِ)®O¿ï¦€g™lMAGNbcuPMN J1823-3724?á°"Dxî?ÉF,)K?Í͛œÜ¢¶?Æ+b*'×ñ?ËqÛOœ?À¾Nôsž¢?èq‡·ø\ü?Ê¢uzeq?¦!KûÀ¦?¶ÈçxÀH??ȱLè¢'?Æ¿€|߃?㸰ÁÊp?³×"1z?̶ΦÊ7O?±‰v˜°?ÄfnK.žñ?ª–ç´(?î™êG#Û?˜A³âëÔ?Šyÿqûõù?³2d.½S?Ÿ…·d…»–?¦°Æke¨?Þnäú–À?̉ârâ†Ú?ÍÕ?¾mÎ?Æûµsûát?Ò¦{&3gÙ?Ç2ïŹ÷Í?âgý‹(	?Ò
5~x<8?¿aj"œªp?ÅIªæ?†ö?ÓXƒ`…R?Î,Àþ7~?ÞÒ4…˜°»?·3ß«v»É?Ó»Ò`íM?·s*1uM?Êãò5ð…l?°WtXõî?éQç)€"?¾ï‹,ˆ8?³ëƯá¶g?¹_¬ûۉý?À€•?±K–âAƒAGN4FGL J1823.5+6858?Ð	`'x#c@;«h¾/{À:(ðzPþöÀ<oE§©ý•@vb)?êQ?ÿ…C5ßµÞ?¹Ãy'çI?Ðît1Žî@«>o§X?ûê"Ò/¿ï@)æÙ?ݤQ¦ùT¿àþ3ÂOEc¿Þæþ¼³úï¿ëüYýÍJÌ¿ïÿùµc#¼AGNbll3FGL J1823.4+68577C 1823+6856?ؘø³Ê63?ì}™UH~?⃵bDe?ÄôòäA;?£eï?"VxœCÎÿ?ۗϾÞfl?ÊÄW䩞†?Ýݳ`%jÚ?ʾÓmƒn¾?º)óƒðºé?¬K»úžj"?ÚÂÆÒ?†?´üHJeŒž?ݏWL~D?´ÿ%s›Çá?¾·‡…ׯ?¦ámÆ%@?䁫"ä¼ê?¤¾%´ØTä?Ð|e»4À?£§•ÿ²Ýu?ºìá²?'EHßlã?Åïf³Eñ?·ç=%UM?é)¥<(éó?» \ýî*?©Yî¦ïÌ	?šˆÚRer?ÈÞiœ5?Ä?}#AM¨?å¼½m‰Ed?È«c¨h`ß?À.¡F>Ü<?´¨	Ð!?ÌBÃtr?´œé±ê0P?帵
/Ñ?·ÕŠ'?¾"³o`'?¦òå†Ê7†?ÙZÂÜç´?­²ßSÌ«¡?ەbÙ¥3'?±SÀVÓ¾‡?Æ´'æ™t?¡hì'XðlMIXED4FGL J1823.6-3453?ëwé܅°À#ß6ï€UüÀ8¦}¢ÃÀ;~ð=ë@ça•q@à?û(œ6,ø?§}–¦B¹?«ß¤jØæá@+Còž@û´^kñ?ç$çá¦?ïù—02ͳ¿Ö[œ¾'!€¿ÒŽ"&±¿à_ZοԪÂ@ÆAGNbcu3FGL J1823.6-3453NVSS J182338-345412?ï§Åç«J?%çȵ??å¯*îŽ(?5­9Žµó"?…?`ÿNs8?~Rüæz[?ïluN‹©A?—àQRǽ?Oñî
ø®x?[Î,Ç&ü?'qÆÀ?–к/JÍ,?î¸3Ë^ª?˜Õ/"9ª¾?v´éϏ'W?€=E#äI?¡¦&¡B6?•›§ò¿þó?îÅ0îÊ½?LÓ|n,…?x߂¤8Ä?`¬ŠúOÖ? 'Ħ+±?¤Vâëí+?ï"
½>²?"p1Ï.G?Y÷Û% '?Y+Îf]2²?šʬ=¤?'Æaª"1¹?î‰¶?¯:	"K?f'IZER'?{'dfÉó?¦ª¡Ñ6ï?®(܈¥­.?î
5WŒ?Ÿ	³>"¨á?zãK¶W*Œ?ƒHîû-¯Ò?«ÉÅ6yo?4žz÷9?íͼ8!{ó?–<<K~¼?…gä#+?uˆh†‰–÷?­Ê{ÂKÈ?•
°buûAGN4FGL J1824.1+5651¿ã<ߘ<³v@:Ù#d»À8w–Б}kÀ;ÛLg"t@½vá³¹«@o	R
?žöÐ"äþ¿?°'²o~h@§Ó[\G)@k#Bû'S?Ë%=|7^¿ãT"Ö¿å¿ž ß¿åÚÛo›ï¿ç!ueݪk¿å#slß&lAGNbll3FGL J1824.2+56494C +56.27?ïñìÉ ?LçvtÞ<ò?7°Õ
pD?(—ÃàQŸ?Vø&›3óY?JHzfíž
?ïÉõWS?u€÷Äð?Qß@îèü?YôtÒÖú=?v­'M°_?r&4Á)ŠÑ?ï´9Ø`K<?vƄí8Ë?Y)kjþm?N²Ëž	0?‰zƒ?u]c}?ïç1= Û"?Iï p×ñ?Mž; g-?4† l™$–?ag3¡ˆG'?CH6ñî
~?ïáz;ãät?dèc"˜•?>ÿïn'!Í?2##ÛÂÆ?j¥Æ5ŸmE?cã++"}¹?ïoį®6?"ûÐ@UÍÀ?aO·Ô¿HÎ?p¡¦Àâög?ºæ!Zä??'ÅR©÷ë?ï^U€K?ëA˜Uë¨?c¶gx'¹Š?a¢A¥¾c?'¾'ý¸âf?Œ¸"œß¾$?ïÃ5ÊÅ¿?guL¥x‰¤?bØr‰µ²?Rªëeí?tøác–Ø?bœÕ$AGN4FGL J1824.5+0107?ëìâ8fE@ÃX¯Ä~À8äB(™|=À;	‰H¾I@.<<œ=Ž@.—eóS?¸Ôž}Y&?²+
Ò&?ô~žš@*êëñ«)?ê¯+ie¿åù	p¿ëgV@S'3¿âT	×ð~¿ë^*Ã") ¿ß&a"˜ÏAGNbcuPMN J1824+0104?î¸LFCu?£¯*H±?i؆]ˆ,?c­®Œ¸e-?¢Ý³9}Ð?£1anQcÂ?íå}6غ?­ý–{#"6?j՛#Ƨn?r©ðöt?¯úÒìi?¬"KÆÖRW?êoÙí̺?¯3…5	?œmË*Mjô?"*(,ìÐ?²Þç#¸?­Uúç?íê,·îï?‹³	"bÙû?{²äPo'?`Ѭ`À½?­o6Ôv"?‰ôz&;òØ?_?§¼ùø­dø?qPˆÝJz£?iXU'Úç?¬JCmƒŠ:?¦å¸Ó‡Y?êðz΅è?Á:ˆåÊÓ+?}Ü2•.s?ÃJ©Cù?ÃPÀêúh?Àˆ³á?êqnŠÕº?®à"vÛê?<Šâ~?–q´^}?Ãöº$1@G?«Ûä¯Ññ"?꒞"Äâa?¢—ÅÖyÎí?™y,tyºÜ?€$uð8?†`,^?¡ßûšÛAGN4FGL J1824.5+4311¿Üý³0æÊ@6ׅ@FA-À:Ô{bvíÀ<+¼FlÌ@!4Ö½;ŠE?ûÇ(-E³h?ÇWOGß=?´àú@ÎQ\?ð܆Ô@Í:Ó»~q¿è¿!Í°"¿¢I÷<Ynÿ¿æò•^KË¿ß!š•m¿É¦hßè]w¿ã•õôVÿAGNbcu3FGL J1824.4+4310RX J1824.2+4309?ﶸbKhx?væc?E'ì?3\åÒOW—?f/%†É?v"ëÌ@±³?ï û«©?†œ7Ü6?^$å?dcîH;?"6ÿ,…Ãô?ƒ7wԍŒv?ïg/.ŸX?{6¾Ä?^ٖ‡]]?J i¢+°7?'/@¸Áwæ?yÝ¡ÓC?îñ6Â[?~®VK-~R?jì¶-ðDs?T&FÔF?ž{§¶ÕÏ?~ïf
¨Å"?ïZn4Tà?ŠSގ/•?Tã°ÁV¤?FVÕ"è?"nW):>ž?Š$ú{Õ»?îâᡛÎ? åN6ºiW?n<Mœîž;?{i5ÊÑmÆ?ŸÜBZn?Ÿ]"©?îĀ²ý³?Ü%6C©?f¶T?9R9?`b©5Í{ ?¢L˜ýý¹?Œ´WT®?ì¸â³z&ž?›Md Þ>?€¡n•!?s‰‡Gnhè?¸$Éøèj?œ
@–"L'AGN4FGL J1824.7-3243?ç<"—Ì1iÀ"V,UÉ`1À:­_ö	ÜùÀ<"Ó~—¶@?8Aºàf@O8œÿ¨?ь®¤˜¦*?Ùk¯#c²@	ŒªZ±ý>@Ùúf=!?ïʇ½ùö&?âtÒò¿â.ÂöŠ5y¿âcò¸ï 6¿ïôcê‹#µ?ïj¾º»RAGNagnPKS 1821-327?åjÙíið?Á>øEB÷™?¸,AîB?°ÜZ%¾À?Î>wÃõ§{?¼îñ ýÍ?áŠÖµÙÁ'?Êhow~‰?°zCç+4ò?³³§#$ZC?ØËÁš¼ö?ÇÇ<úm€?çm\
±£•?°ŽéeªkÞ?·­¿Éâ•??¢¡ê¬å?Æs¯ðH'?§ò€}£JÇ?è邸Vž?¦<~xÎ?¹ÐMÆîw©?›§ü14™?¾ãœv\—t?Ÿ²(῅ä?Ù_ð´Eü?Â81ñç?ÆÞU
svo?¹2Lёn?Û0äÇÈߋ?¦Ì-Ñ°?ÔͶتâ¨?Éã9±ã£?ÂWƒubO?Á˜æ"U·º?á\²Í6?Ì31™¼:?áÒDsªû?²ÒGâ4›?ÃM¨ èOW?«ŸWØ/á­?Ò´£5â?°­WzÈð‹?Ýïr¥J8?²'ÛÑ4
?Í3ܬÏèq?³Gn–÷?ÓvŸMÓ¯?²¶°Š.¿MIXED4FGL J1825.1-5231¿ïn¨ö¦1À1u;÷'À9N\(õÃÀ;ä(ôëÐ@_êVËhÊ@;šû™hò?°Ù·µä?ÀªqK´´@Òµþ,Á@'dkåV?qÏJ*›Š¿ÙÀ.XØß*¿æ¸÷˜Rq½¿ãõՅØò¿êC7¢®–+¿ïÿ ºöAGNbcu3FGL J1825.2-5230PKS 1821-525?ïâ^QøxÖ?[5"PMw?RJŠÆk!?FÑhÆýWœ?d|i2´q?UŒâÃ+~?ïíÛF¦ò7?fhᏭT³?2ʳf1¼e?BØ6ÓOŸ?_–Å–Ý£?cµ0hp‰W?ÓP[?"ꚢŠl?oüÒ(JY½?tFÏiT˜a?‡þ›}©¶ä?'êŸWˆý?ïèŽó£P?H†-SAš®?4´¡gN}?¬ž¤è)l?eWÜåèŠj?GÇiñ?ïºU‡#¨Ú?q[;Ì0"?gT@kwi»?\ÈGV©£‰?w+;/Ž?kXèµDʧ?ïÎÁ¸¶Y2?}õÄp
€Z?L7¢©3h?cUäøåqñ?u/j_?z±CÎCÁâ?ï<9Zó?F°î"Ô°?~ó¾;'´?È©>»¡?"{«Sõ-?‰"S0ˆ
?。ñ&?iõuüŸ?OF¬Moë?@^)$'-?}"Ù×óT ?gÅ÷¯È.ÖAGN4FGL J1826.0-5037?ÁÑüfsÒÀ0Ý\…<ƒÀ:åCä/À<LERðh@ %ZÕHœ?ý͘T<?ËÏ?tN†?Çó(ªB?ýÒK&nÿ'@ݺÄâr¦¿ïþM"r›©?ïÿöÅĚϿ¬&SUȬ¿ÞøC¾EËf¿ç]þÈs¢¿Ñ‡wã¼RAGNbcuSUMSS J182551-503914?ïâ'Ü¥¡©?Z]>À2?BÀN*4g?8¶qÜ8ë?h¾©?X-Ë}1þ?ﻬVÎÞ?öÑŝÂ?VÅê#'Ž?_YŽÝ@?|¤†û»Üg?qï
9¯?ï_à³3ž"?"^øÆR&?qlR³³ûŠ?y€æ_é÷4?Q©Ó¾ýƒ?€\ºTJ?îÇ"èœY?tÑöÿdc?†(ÓOÊ ?\¨zÜ4â?Ÿ:¿9rZ?r"Ÿî'?ïÄzÕxå?r[T" Ä-?UÚ§W$?JÌk'?xKëwÈ˜?qS܁?ï?G1Sj?'ÖÌ;=©ë?nB×àŽ
?{mÑÖS3±?"N¾Úân?'<"æ¡ï…?ïSßz?‰ü]®èÓl?s€3j³K ?y.í»)õ?˜H«­|×?†s^¶2›?íLáùÒ?'ŒìÜ
'Ì?Š™á–r¬?sËM®¥ ?²L#¼j }?0ùAGN4FGL J1827.5+2015?|›êΝa@,X–Ý&·$À:ãAÒ2g[À<K§°³''@ N+9>ºü@	T!ÀD(?Ãߥ+Ï¿¥ú—$82e?ã|‰ˆª^
?û9ÐUîI?ïü!ƒÞFr¿å(Gýo¬á¿ãœa?`9¿ÚÑR+Sk¿Ñxâií¿íC·'sAGNbcuNVSS J182730+201309?íÓ¶P^'2?±!$ölt?‰£ "äÈ?¬ªu7G'?¬a2.'G¹?¤P¸«óG?í#ÙÜTÕ?¶;ýî#ý?€üŠ¡¤k?"ØÐJ·‡Œ?´ÁŸÇ˜öÖ?µê¢ö?š%õ?"Œ7'Z¹t?quAУԮ?kdgq†$?¤—N!q?'ùèӂb_?íÒ	Š‡?ˆK+JÒ#]?uÖFËyç&?\£€º-ðu?°ÃHû­?‡ÔZÑ+?ëÍÖÑC»'?¶(õš/óa?'ðÖCÒhq?–á0ÈOª?¿3.«}?µgpR}¯?é\åD?È 0Ý?
!mbi?›Ôܐº!ú?ɬ頠§ˆ?ÈÏ!!?ìš
¡Tà?§Wœ´¯u?€|HïÓ?x·Q~z®?¹ûj6X?¦Ž*pYó?éWê,"|?£M%Ú|….?JÆU·?~†àIûM?È«¯=<Bô?£¹ËP;{AGN4FGL J1827.6-4029¿ÛY§ï¦I3À*Q´þzÀ:Ås½fþ<À<Nx"PŒà@Q†QŒ@njCoÁY?ÐP¼›|GÏ?ÝaÅÂÂ\Ü@
•"äþòº@Xâš>…?ïùu'
5ô¿çumjf¦'¿Önà2…8¿îoÝÞm¿éÏÅÀi<¿ïÿ®¡hšôAGNbcu1RXS J182724.8-402904?ì·;CUÊ?µ'W~«§o?œAU"N«?6Bõ,™?³5åÏ?±•¢0os%?ì&!¾Qðõ?À™š:©I:?¢iã›áÁ}?®€'T¹†B?µš?—œ?»-}s•›U?êµ½HPj?¨k÷7îÿ‰?®¹A§‹É?žÃNÈÀý?ºõtÝ]ÏÐ?£
I"žˆ?épÎéKwg?–þHܘ?ªy7·Aï:?‡$ʅaã§?Þvmoš?"*¦û4œÈ?èö9üÍî?ÀØÔh³®Õ?±¥]$ Û?¬P'k\W_?ÃT•â¥?»>æžô¼?ç HýÊƍ?Éåf@üŸx?¹}lÜ/ý?½©@'ѵP?ÆÀ%›+PL?ÅôA¨8e?ç†ò›qÅ?°íVB~=?ºÓî-‰iå?¦·ý"f?Äz>}œÁu?©t×î>©?ágðì6?ªW3²Mß?·ƒ `)­Æ?4Ð.¨ ?×H^KÃ?§‰
V/AGN4FGL J1828.0+2634¿É덣
®@0ŽØ
±À;­î»4À<Žä†&ö@ ¬!®{}û?þ»ë¹!^?Ð ‰ãC0×?É87)Þ?ønã]2
>@¡€\[˃¿ïþR¡ªˆ?ïãë¸J_¿À®ŒDòMe¿áp ßs˜~¿Õj\|ؙ¿ë§A"4ØAGNbcuNVSS J182756+263313?ï£èx,•?xߨß?:²?_u™`>ÿ!?SO"{f?ƒ.Ñiá?v"Íü?eŸ0?Œé{-Šâ?bgÊÂðü?ewÜa—Ð?‰›L§A…®?ŠÌ0 ­j?ï3µâ>h?‡Z™BuŠ5?{ð'ßN%?ƒ[Kh#Îé?' $•dw?{þ¸nOJ·?î£Ð0Ha?{L×}o_?yÑ:1?^ ÚŒ›1ß?¢Ÿ¢ÙD?z­8ñ¯În?ï+nþ1ì?'€U$õ'Î?pfÙ͗4?e0AD?–xi¾Í•&?é¥S>Ê?îÕ –'
?œ½HæÇÌ?w7Ú>$ÕÚ?ƒ—y²Ê?Ÿùx2ˆí?—瓳·¹&?îh7o`"œ?•ƒÇl²þ?"	kw<"?†w´þ‹?¤z.(<"?'b£dþÅ3?ì"áBÇó?•ì_Äs¨g?ˆÇ›9˶t?vîóšÝ%?¸@'†ð"?•[½)AGN4FGL J1828.7+3230¿ã&wÊ@2Ÿl‹C•À: jüÎÀ<§Iˆà
ò@Í+4Ja?þyŒcP1q?ʜuìì'?äk•ð]Ì@–fœí@`Fë¡Ï?îé}'Ô?¯ ®ˏ¿Ö;™Ƚɿä…Lò!¿ïÿþó…õ?ïGÉÃ-ÚAGNbcu3FGL J1829.2+3229B2 1826+32D?ÚÞáV
'o?Ì(e¤Êz7?âýkÙ x?Ìë½ +{{?'Ò=''f?š´±àÓ¹?Û½+ϼ–I?Íùý{îZ?Ýçò ¤ƒ?Í-»ö¡îŽ?¼Ë°ò?'Õ?´o,N£¸=?×äÞ¼½'?³â•¯3?à¬ì÷Sx?µ"â*†?ºW MRn7?¤"͹Èr?éã¨`ܹª?£$}ô¸ð?¿^Êêä(Î? tM™`Å°?±ƒò~;æ?[€
O¯Ù?ÓÀ'þéj?DŽpM×	£?äà‰Òž•N?ÉlAS©Â©?£óJëÚ°Å?¦)P ã¸?ЀÜäœø?É(B2›?㍆ױ=‹?ÌØÉ"q?ÀÈ*Ø—?´…À¹Ð
"?ÒPþhXâx?´•ÐŸ/Õ?ãœÚ¿6r?¶Èü]´=?¹Õ1ÜW?"?¥¶ËV·é?áBl¼k֓?²°6S6#w?ÑdYœå£?²çÐwì?È-™Ò_Äó?§~dd! `MIXED4FGL J1829.0-2417¿é©Æx'¦Àäœ@=òÀ9M	1´®À;™Þ˜§+S@˜#wÔM@´¶býü?³ÒŸt¤í‹?"³n#kŒb?á Ϟ8dË@¼‰¿±Ü1¿åŸ'•¿†¿Ú##´e"¿ãhÆ]Gô¿à6U\Rç.¿êŒÕ€Ðtø¿š ½R¡ÛAGNbll3FGL J1828.9-24171RXS J182853.8-241746?æë áÑ/¢?¹O'~6+?€è´"c«?s¹û«é·?Ñ¡~?¶N?¸Îqj5ì?ë%/Òüš?¸}ʓæ?f©1§î?q/+Æë&ù?Ý9¿Çß?¸ÿ×Q4?ë´Zù×?¥P
è
|?"ïÝöÈ?Œ‡z9*cÄ?½!hgièô?£Ÿ\;À•?í¢YÖ­m®?‹-H!é?€þ¿š~€Â?`çI€G¨&?°ÍYW½´µ?‰ˆšçÏ?ޝ@xý(?Ã*ä¿ «‹?"顏ta-?‰¡c‰ß‰µ?à·<©?Ã'Î_7â´?ãÆîlëÍ?Æ®KjÀë?lÕiˆ¶?G"qKŸ?Ø;ÚxÔI?Æ«YPuº?å]N!¡…?´¿cMÝL…?¥Š'FüúÎ?—JyQÎÊk?ҔÓÞA?³ÊÈ|xO?éó)\3¡\?¤›ŽÐã"Ö?—ÍFâkT?€7íÃĐÀ?Å9±´dîd?£È:ØWMIXED4FGL J1829.1+2729?æ}®K"­@0²{åS¬OÀ9ÄP¡C§À<L¥ËD@Ð<Q¿æ4@"îV,\?¼MfÿØ+¿?Äj´iS«¤@¦Ôš÷g«@ã·Shݺ?–tP›	Aƒ¿æ|š…R¿äñržƒ
f¿é¢>Çç¿ïÿ#–Ýýw¿ïúÚâ9EœAGNbcu3FGL J1829.2+273187GB 182712.0+272717?ï$
;Ë»³?LàÂó¼?æ£48pÿ?…$ޖ)ËÌ?‰Íß·Ú#?€Ò
­€j?íø´±ó\?±08Ýx2ð?žº '–?§ËÅsŽ®^?¡­áC4/?œïb—Ý~a?îÀ'p?"t±xu—
?‰ÖgIH?‡tBÆCÞ·?›ÚB.¸J?ŒVÇ'•q÷?íÂo™@z?‡'ØÏõ?¡8~æ[[?€O$o9ãj?¢ ˆGÍú?zLÑ/)-·?íB-]A‹?ªØʨw†^?¯B<xqÏÓ?¥˜Íæ¯^?žóAe+üÿ?–&R‹Ncw?êû1E)ç?ÀþÇÊôd?³:Gí\?ºˆâ
E?´ì/٘l?®3VVw&?ì€h½{›?¥»#e·t3?§}1[§!–?p&ŸAC?°>!eå¾ß?˜Ë°kbç?êX""O¼?¡›‡ÞÅÃz?¶ѵìÛ?œ"¸mÌ	¤?·0
+·oÂ?"è0öÕAGN4FGL J1829.2-5813¿èå	trîŠÀ4j½ãû½À8†‰À;–lÅ%8Ÿ@­ŽE'§d@rÑ®³Ý?œ€4»Í?ÀXƒ#á\@`^åh¥@
t÷"ᬿÑAwcä«ç¿ãÆ°žBö ¿èS]õÿv¿æë+Ý~uÒ¿ìIìqþ¿ïÿî' ÇAGNfsrqPKS 1824-582?ï·t#Ï?wá•z³Ìâ?pƒ"BJ×W?m¸%ä~¹Ö?sðYìEé?k/[¢ê‰?ïãß+°C:?pGír¾GQ?;¤®œ+ôÿ?IÅ¥9r?h¬>¦õß?mÚrI—ýN?ïCfZŽ'1?"= Øù½?‡"
úzõ?‹TŠ"†?‡¢^ê:(Â?‡fcc•?ïó•¼mË?DÜÂþÑï?4øg
?(ÔúOS}ã?S–†Ð aÈ?AUÕƒ{ù?ïªÈ†þ·?~ªåž	S?rvŠ²^$?qËÁËÄ?x%1ë?r&V¯q?ï²yY)´Q?ŠMÍ/W¸?Z9'p‰¹?tñAeÃÜ?€ ¢"Äb?†ë˜ÃDˆ§?ï
=¢š@«?•òPac¿?Žlõá=ÿ?Ž³M:iŠ?ŽC¡{¡r<?Œýº½˜·?ïÕÐÒ*?h‹—m"3?SuÄÈ/zà?JÚ itŠz?p:%Úø)?eÞ
!0¾AGN4FGL J1829.3+5402?؏üöôØ@8Ìñ`®—À9úVÔ"+¤À<d?³t63@ 5q4ˎ´?û©Ø@žUÁ?·*KØñsJ?½Á"o:öK@õM¾Ñb@9{E¼D¿ïå!4y?ï'~ nö¿×—ñ"íjÒ¿Ö9ñ'õèO¿Þ‹}ÂM—ã¿â'«@‹AGNbll3FGL J1829.4+5402RX J1829.3+5403?ïõ !ŒÜa?@u+º¾¹V?0û©Ë+­‰?!(ݽ¿TM?P€Ò`½a?;`ïnî.?ïÐÕ·H?u5$‡8à?QË¿''ì‰?Z—Æ'lp?s"‰Ýƒè#?pFÃî2ÌQ?ï½Ùì^Ò7?h9ö4Å?So5 ¬ö~?@¯Q»ã?|7<‰'Æ?g9:Ï­Ôn?ïjÁÿ-6?dºžiêÍ?u͔,y.
?S,äêAÔ?Šh¶N}?a)lÓ‰+?ïìË]ë?Psø:Än?Bc'àõxò?2'ßßxr?]7|Ôt†?Lc¡'ã'?ïxÅÿÜ¢?‹ëpnŠ?eM@~	4?og¦Fï]?Œª~QT;?‡ ³4èm|?ï—4b&¼?rÝñø'[ö?]çÀS€?XÐo~Û?†v"¼{?pH¿Â¼=?î¹Ì_È>?€žJ°¶Â?†+ž-@ï£?nšV¾_Å
?°¤é}t?z
lü˜AGN4FGL J1829.9+3934?ÍI"5"F@4ȕá~4¹À:Ðw/†FÀ<šã'áït@HK×Cô!@"ýØ?ĺ{B?·ÉÓH<ç?ôÿ5ºÌð@ê;ò•í?ð¿ä:'
‹þ¿å—Î=e;C¿Ù¦DÉ]­¿ë&i@‹`q¿ïånN'4KAGNbcuNVSS J183003+393638?ïghøùÖ?¯n–ÖQÎ?c=‡aÁ?[ºà.ˆ?¯™.fz?¯e;ÈFïí?ï8ÏzÀÕ?'Y/Y$'˜?wý€º ³h?xÑ'hÖ?'îåë¯s?ŽN¦ÉÞè?îu#ès²?–,ó®,"?z£õ–"6<?{þ2¸s€T?¥YBÎr•?•=ž½O6?îw×U´4?}5¹"Í?' ù& gd?mƒÕ
>Q&?ž}+ìñD ?x–2פ´X?î¸ZáTI?¥s˜›E?tùSA´=ÿ?jWŒ˜Òâ?¡Û'†V¹?¥B÷Â?îzñ?¡xeңØ?ŒGß®m?ŽXhôÝ£?¨v`$E6?›ºQb,Ì»?íºâIê7t?œøžÌjo?'8]2@à?€'MÛ®#®?¯ÃÄ%ï1?›*• ?ë¸ã‡?"'Û¶ÔÐÃ?©úpö˜?‰£\[¸œñ?µ¾¬f{ê?'@G‹o0AGN4FGL J1830.0-5225¿ïS"ӝ\®À2ÁLf
À:É20Ô´"À<lý@´%@5ՈJø?ùÞ Ô÷=º?Ö%>}êª?â¯'9*Ä@Ü;\Í`q@@DˆE?íº¬Ùè>B¿ïÏÖÍ׏?î´ýØÞS¿×'Ï<h¼¿ìCÌÞj"¿ïüDôü–¿AGNbllSUMSS J183004-522618?ïV˜‰â?¢~g9ûq?qÖVƒeU?t?Ìi¿¨?·fŒ—s? oæn"Ä^?ï0ºe/A?¡Á9Û=ßÒ?}'gK•·?˜u2¢µÀ?'"ˆDæ?–²<oöF¿?íCŠ›úÇÝ?£?‹#gÁ¹?ŽÆ±©üU?Š™–_??²
ë	†Ž?¢¹¤¥1"?ìæ_d-já?™`ñB´Ø?áàQ±Dþ?qWæz)³?¶ÈÖNU?˜ò,þqÒ¯?îjÍ¡¼†a?¢büò«ïã?ŠÚ÷æ^¡Õ?†E»–±—C?¢œgè<{?ž®W?î!xöu"?±²Næ'ҝ?+~ÿ|†ë?¡®€@,?¥Ò¶£n\?©þ%½ÝNX?ëÝý¾©•Ý?«/is7å]?"½/îñj?Iæý_Œ?¼ Ì=Û­»?©§r/©X,?éäDa˜œ?°ZÂS®3?†gf2èI?rõ"‡>?Ç
XJˆ?°Lé'=J\AGN4FGL J1830.0+1324?ÈóÕi˜9@%~`ÔV.À9é©óƒð»À<	‰±Å	Š@Ä{MSDö@SZðç^?ÀHjýÏÏ?±–c?{§'?ôúkÖ证@	€ãäky÷¿Ø´ªagùä¿ê–à·e\{¿à'mb*W¿à,&Ïw¢¿Ý:¤OÜ¿è‰52ç³ÙAGNbll3FGL J1829.8+1328MG1 J183001+1323?ïØ €(.r?…¿ïÄ?AÑ.Â?LçÑAû´?q̅í#á/?ƒgÀ°OÍ?ï†þƒÔû?"(Ëdé?KU0OPdº?W·ûlbù?Œ‹(d8"ä?""™(ò?ïy#Hj¹?'T6©+}G?]\òsIS©?W)|'â?Žù"¯?¾ÒV+2A?ïI)aÂÁ?l顲(ný?Z»†‹c'?7֖c?•/{¥u—?l½ÔædŒ?ﱇ™UÁ?€[œÉzãñ?PJä'ü½?F}êPü»?¯"•H£?~èïý-Y¬?î®Ó°Üá?©/&KRÀ•?a½l]O-?r±|ý{Â?£öî9}%û?¨VÞhh°?îÐyî61ž?'ö"PXf?jõnOÀ'?i›‹²¶V*?¡X1Änš?'wú-EB?íÿôa¼2¡?‰sów€Î?pãk
—3?WYeÞité?­äL'P?‰Da-íN"AGN4FGL J1830.1+0617?'OÙ£G1á@Wáá1àÀ9<•ÃKCËÀ;‹PMö-@qV…sÈ@Ž£yè#?¸´¸ƒê…Å?·ÎFO?ü#ûØSÍ@z$n?ïÒjeÏg²¿Útî¿eÛý¿äÎ×ؙŠ¿âHŠèü®<¿êÒûºöás¿ÜÉÇÿÞrAGNfsrq3FGL J1830.1+0617TXS 1827+062?ïBk."|?†zïU%ù?R_93mä·?Cc‹L¶–?–Œ¦¤ÁD?…ä¶2^?ï|U>ÜðÃ?šÔDÝ¡þ?Dš²Úé¬`?W^–$ q?¡ÌÈ?šžÛȟ?î}Ø€'z?•N®¥¦í?Üԍ#ª*?
7+&}¥?¤&å
?"A6OI¾?ïÑwu·Ï?Y´Ü¡Ç1£?>)ïs[?$øc¬2Z"?ud"öAhÀ?XÏ­3–³?î"2³=Û?œ2¡…#Õm?_¦áòk?RêÀã"R?¦Ä'—È©À?›´ì>:?ÉJ!?©åt•Q?TÍ
Ñ¿vµ?d'£ÁyQ?¥P{7½?©¬½nÓâ?ícÆßî?¡Ïìˆq+¦?Œá¾ëE…\?Š…Ù¦Øz?±Kióª*b?Ÿª/)hx?ï|)L2;D?x¬V-ˆÍ7?VÈ*ÍÀ+?Eãûž%Ä?Ž§µÎôé?w¡¸jøÃâAGN4FGL J1830.2-4443¿É¢¯,}âYÀ.jÞe{"ÜÀ9BW@X¶À;é·B÷ÌU@'²^Ø(@L~ä­³?³XÚ©¯;?ͨœkÛñ-@Ú:_w^Ü@íÇBŸ6ç¿É6$ª.gG¿àG¯â0aG¿è¥ú?÷'Ç¿èeÞfRD¿í`b@fø¿ðAGNbcu3FGL J1830.0-4439PMN J1830-4441?ï˜É|$,Ÿ?€¾™e¼§L?ƒÊb¦ž¨ã?{žÙð&?hù:y… ?a=¨°Ïro?ïëFƟw?lè¥\yµD?2ÀZ0»´?CÒÐöýZj?ba-ôÝE—?jï"Íc?ïц¬S?'"ª€í\W?GzÜÍÈa?ªç
¯…?bÄ­×Z?ˆ‡˜ÖŸ5D?ïê¼,I<½?FÁžÿ€ë??úL½íé¬?&²·íS•R?aD‰æ«íš?CâLoM´?ï81ùZR?¹ÀfÉý?'òBÅu?Šâ×Ýo]?|n̯¥-?t"v3Så"?ï̺"²?€;íà!w!?HàøM—áÞ?YkæYÛP?vã"[¯?~W1¦Qt?îM•.ÐÍã?¥&'&bß?˜.6ËÎ]?"–Úy=?ž#b®ì?"¬ÔX4?ïÂÜ5Aø•?gútwFl?X
1	A(?Hi=—ßò‹?xŽ™")Z?dœü°Ù;òAGN4FGL J1830.7-2713?ïúÂå~…¨À"jP
_À9—ìoîÀ;¨uÕo3@nƒGr°@b¢§_U?º¶ñ™4ïÌ?¼Ö€TÏG@<h€òÙ§@u•ßû¨­?ïŋZ;µ¹¿áýwå?¿áýÖ?<Uò¿ÞÊÒ É¤#¿åÈ¿nÀR¿ïþ؃ªDAGNbcu3FGL J1831.0-2714PMN J1831-2714?ìir܅@`?³×gr?v2Ù§ÁÈ?z®	Þ¾ h?»Luíu—d?±Ò©"^W~?çãGYþ?À_n¾@K?HJ0$×?ˆ}P[䷍?ϓîCøÈ?¿ÂþÓì7?ëö˜ãÄ?£tAÀE©"?˜g0Ìâ­?ŽeoÆaxÁ?ºEŸŽ¦Ì? éÆ¥èȱ?êxIˆ	N]?'óîH}??§E¸!@®?~¼iœZx?ÀM•2	p?€z$8s?éžÞ§ì?¶6þœí?Œ×JÄ?¢b)c¦A?ÈB‹Ø]F$?µm¶³ý?à$à³ù0?ʂïÇVHë?£kº'<b?¤¨@Øi?ÝHÇT<î?Ê@Ô±r©?èfΨfˆm?ªÇ'ОKW?¥Ù÷>T?"ýÌy3ÖC?É#Îà½x?§æöÒVdì?ä3Ãä
?£¹¯L?¹™5E²ß?"—Ÿt£6?Ñ2,tÊy®?¡[ÙØAGN4FGL J1831.9+3820¿è¨éj‰®@4š€If{À;Pz9'ÍÀ<¾Ýšzj)@ cnv*S¼?þ†Ôš÷g«?ÐFðù²?Ð2?"?ý,©@։å@'ԱÿîÂë'D"X¿ëöòoô"¢?ïþž¦ž»¿àԄ¡ºÐK¿è"PïܜN?˜bãz
b>AGNbll1RXS J183202.2+382132?ïÁŠ¤^C­?qpSc )?[ëõ[:?QÂ)ië¹?x?°›Éµ?nÿ/Ñ8s?ïXvؾ6v?Žû`'˜ÌÉ?sK>8KV?uJ\PS?Ukò`h?ˆÝéñ	?îÜa·¢e'?•9tp^?p–$…="?r‡Ï{؅i? '!ãʤ?"­Nƒûà?î³9Èùƒ?'UBÙl¸þ?pÝW–å>D?a:©š¨ÃD?¢°¸~"E?§¶öæÃ?ïcv«qÍ?‰-ž§S>?qe:»×?gI{{?Ž¶/¿oÈä?†"Vš§œÎ?î~D÷Uâ`?¥GLGóV?€w¢ù¿Ÿ?‰C2Þ
aÉ?£ýÇÏ3š¼?£*–(ñ?íô¶~èÏs?œFbt?yªGÍ+9è?vúh XÅ©?­Omɕ?›™£‹¨Ë?ìWlòáMQ?¡r†E¤?Ðþ…5šP?}gLS¹e:?»
x˜±Öì? ¾	­¬4ÍAGN4FGL J1832.6-5658?à"]âM+qÀ4m?ž{À9d8F˜jÅÀ<"a+"@qƒ¯½@"+¶g/º?±œÅžbe?®±±à¯¥?ú*M`Ûâê@ÙFœF?ì.¾¯R¾¿åt…
›¿à4º-ô¿àP"AÉN¿å<YjÕa¿ähÁTɅðAGNbll3FGL J1832.4-5659PMN J1832-5659?ïÔÏÃ!R`?dÌéö{äQ?Gþ>ýŒ¼?6Ô`'Xhè?r·¾"f3B?bíWŸ4ÌX?ïŠsX^³?zªµoëÏ·?T[Å	•?\B¡ÕC9?yº¯‹?Ü?v[¢p4s?®œÎ?rƒ÷Á¤ú?]á¬Ê¾ ?`O1QÂш?…2Ykª?p"þ½¡¿å?ï
'XNíñ?tšÓ"JÜ^?ÛdÒT¡?_Èþt¯;W?•À"Šè}?pÖ=¡µß?ïœ,üéf?|.KE
d ?_‡n
¬ý?Q.f1›?…ðlúè?y ðU¢?ïL"ïØÚ?"ßMu,;˜?i…zv"X+?s¡#VìRÓ?">Џñ¹?'¡íA6?ï¨Á÷þ÷?"Ä•BÅ?lîöSr?päBïÈ?˜­#ՖK¼?‹Ô»È\i?í–wj<+?ÂÁbÔR?–ËÇY¿e»?xš,
zÐQ?«9"àÈ
h?ŒVX9BôAGN4FGL J1833.6-2103?íyÔñUæÀѹ_1¾¿À6`°Å/JÀ:‰"ªNô@¸£Äë¬â@¦v§&J?‹­IòèÔ?¸eúéHÙ@&¬`gHäu@Aóâee¿Êg>ÀZ#¿ãÀVgâ¿çlë¯#¿ç%¼R+F¿ê>ùºì¿îö÷ãÑÌAGNFSRQ3FGL J1833.6-2103PKS 1830-211?ï6ÅìÞ»?œ¹07Ö0#?rx§¬ºÝ?x5ˆ¾y#¸?"Ÿä;GÌ?˜²‰`®™ð?ì
c"õ?ÅZ.A(a?†,ÊîŽ.%?¤é}»Xé?¸ºˆÇ/?ï
;²?ëÚ4òP?©•ó€lF?¨šÆñ9ÀJ?¡$¦¼7–T?´àôôt‹·?¥½Ï~¹á'?ï;Z7j5º?"/é3(?zÉþHÀB6?pŠ˜¿½çJ?'â9…,±+?}Ð%È¡-?í"8ȸ.õ?­ú×ZT?"¿m<¨Ç?UŠ)pÞ?°ÆL	€Í¿?«ù>zý×?é±Ï×i?ÍåWõ4u?•žÉÂçê?©årà8s?ÇM_ˆ•?ÌùÃ¬è?ì>Hé¹þ¥?¨D–Áy¼Â?¤‰-NÎ?œJAMÅ^-?³Æô cp?£ª ¿2p?íé1O‹áÿ?ž#Þ`ÛÓt?'1Sô™¦w?†$2gÅÜÐ?¨TA
aWß?™Üm©¦¬ýAGN4FGL J1834.2+3136¿ìOp2ÂõÞ@13¬)ÜrÀ:˜T+
pÀ<MAî·Ù @!6âågù9?þEäæŸê?ÌüŒ¥ä?²{;4´g¦?çu *­R´@ç™ZÚl?ïêõ6¿åŽü¢}mê¿ì›'û? \¸<ÇÜx¿ÝmmVD°3¿åÛBöAGNfsrq4C +31.51?îõ`<*ӓ?–0kb©P?U‡Ùl/5?G™uÑÛ?ŸûzÞc:F?•þê¬0Êù?ï­S,DN?¢×üf#'°?shõêTÖr?vØ/@‡G?š!Æ	 ?¡>ýË?è^E'?'©­t(,*?qUî\´è?te.ë?£êñ.Üm?'çcÕQ%™?íԆhu›t?‹Û	Zڇš?}̝ÿçÄ?cæ¨\VP?®þ¸}iË?‹QûuVÄ2?î Äöa6?¥€É"5?e›éú]ëJ?`19 Ɠµ?¬™ñöUpñ?¤šxۖ»¯?í˅Ä"†?²W€*Ãß$?€È}ۖŸÚ?‹ýnó³?¯"IñÓ§?±}Fà`¾·?íGGÆNi¬?¡Jaz¨Äƒ?zÐKrrJå?y÷ðb3?´½ü_²? ¥åa¬ÿ?épò…\åx?§taìÁû?–x<F
?‡÷º™0£?Çm3ĉž?§zï¥äAGN4FGL J1834.7-5858¿ï‹¹wŽ	¡À4ñoiÀ:›ËáªÀ<6h¯ìÂ6@¬Bè2@'V¡ÍDÂ?Ð6Ö@hûÂ?И
M`Ûã?þV>J¾j3@	(#á≿ï_jÿR[?ïãyòÄ-¿åF;Šsâ¿ä&vVžrF¿îÚ"ö¥
¿ïþs£eË6AGNbllPKS 1830-589?ï§fŸ­k?{€ãç?cáôK?ZzõN×®?.ÝVí?vŸV…:lƒ?ï¾ç¨µH?}î¹Ö#X?TÒ»w݀¨?aÂ~ýà?{W|´H«ò?y,¾'Åc?îîK´M=å?"G"‰	Ñ?uîé]e?ƒˆêû,ß?™{'ÿmõ+?ý±ðH??$z*5?|Ï1 ÌbË?€Þ1ãe?aöçîˆS·? ðay$'?yۆJÂ?ïC°¼ÔdÏ?Bfê%x?vào+²çn?p8¨4gÀ?'Ñ̜îf9?ˆ¶ˆúÑG?ïS‰ÈsÕ?$Û·D|?vë«°­'a?‡z+.cn?—z£áÑS¶?•Í4ä~¾N?îU/g Ë}?šT1îÃ?Œä¦³2œà?‰™nmÎ?£sßàJº?"þð¹Ð–'?ìÔhùyå0?–¥8GêÜJ?ñ¢/Wk?{È#¶6µ?µ t¥©?"³S"Ë«AGN4FGL J1835.5+1349?í>X>ãô@#pxú½ àÀ:^qhøçÞÀ<´-™–?@xD6¿@M|Š•?ʪ < ð%?Ç­NWPôº?ÿw¶4ÚÓ @ðÓQÌ%ˆ¿ïÞf"‹=?ï˜j$aY¿ãB#%žõú¿ØÏ= ˜ò¿å/¼»Ý'@¿ïúDŸlArAGNbll3FGL J1835.4+1349TXS 1833+137?íõâ‡õt?­T ?l¼/LôýO?bc|Ò
©a?®Öð\ä?­9P^R?ïkœ"ä	?•1f`yjå?Z|é´0î
?dðgD©p†?÷]Ö04?"
+¼—+?íÝ J€x?˜"›Ë%—d?±úæ%?zèec?î?®/Ùñ•]?–"ÕZÎ?2³d?w‡q:¸2@?};àë8I?[ZããÙ›? Î3ûÁ=3?ueÙ½¼ß¨?ë²@/¬&J?´L¦zªJ?îˆP÷?uAJ·¯j?À8êÀ†K?³ã:¯JÓ/?îe`A‰7L?³ÕýáJeÝ?r›‹0}%?ƒŽ‰Í¡'?§hèr€â$?³pi,ª³?êÖgmw|¹?«J¦}"å·?þÓºe?…ê=Ví^?¤K'pM?©‡e×£ª?í/àÜúÚ?'QŠ/po?Œ‰U¦;Í?t­dÃtAš?²ïÎiæëµ?m»Ÿ`AGN4FGL J1836.4+3137¿èéWYë@0ÇQzF<À9ÃÈXÉűÀ;ã'‰±Å@·5ôƒ @ð%ï?¶‡Ü¾îy?žsÚÔ?å£|f'ì@	'tΉ‰?äPŽù,§(¿Ýùà4ì¿á)½h«»¿èŒö%‹«¿ã{6l£—I¿ÒS<}‰ÃŽAGNbll3FGL J1836.3+3137RX J1836.2+3136?ïàÚj'®?b‹¶õҁü?FTAÑm1?9SN¡ºæ?i…3‡9?`pj>îÃd?ï·òJ?yØ<Áv2?T¦'{â=?Yj2gø?Rý z:ƒ?vt€géÓ)?ïe=oÞE?†Ê˯…-?nîiŒ®ø?sçÁ3´1?Žõ	Ÿ•¯?ƒ'Ç4ÛU?ï
…æ?ráˉC÷?pDã?C"?NºÑñþvD?šªò¿‰•?rrjVd?ïÁt­¸Ê?s|0Eα?WŽA2
¥\?Kðۛ3¹Ô?ybÚߍƒ?pþ~£Y˜ñ?ïK,À—#6?Ï
ÁJæ?d®	ì|U?oÇ¢]cæ‹?"¦±CÕ#?Œ69éSíÈ?îÇî¯Ü¸8?"¨k7O…?{ÌÒçÝ?{õ"'…e? "þ<?þ?ËµåCö?í
K'¡?'%|ê¥?‰>ÚjËú
?oÃg""ų?´'ÒVúb²?'báV³7AGN4FGL J1836.5+1948?Þ$9¶3k@("'Ù±·žÀ:#GÃEeÀ<(¢¹ÓËÅ@tˆ$QC@ÖïÞIÌÓ?¼M3y…'?âmY09?ÓÌô9ù ?úJC*L.Ø¿ážf½¤:Ý¿æDw(U‰Ÿ¿ã F&Tþ_¿àËx¤V‹þ¿Þ╠Ž¿ã'¸ú‡ñAGNbcuNVSS J183632+195047?ïVjt+å¦?ƒøbê^Þ?]ÍñX‰?PÓó'@‡j?"UÒaº™¿?'æ¡ð5HÀ?îUœ{eñ?­+•îµP?r'gIÍjã?xGãZ4)T?¨Uëc΢?«zÁÀ<6?îìwJöYŸ?‡Î¯–4ž?täaZ5E$?pG÷¦Y(?7þCô=Ø?…p04ad?î|eÀÆ?ÌPÑf?ˆ<¸\¶?`Ð6½m£?©¶0Vm?€Înë¡ c?îài.9F?êÜw–Ž?wœjs')?fûçm"%"?¬¿EàëÚÝ?œ‹5HyOÿ?ë#ËR4'h?ÂYŒ·e?h]¹#	¶?—ñItu?ÁšLÛ-–D?Á«º{ïî?퍶´²yº?ƒl®€	?ƒy "Õ}ª?wÀiُ2?±#H€r7?›§Wêš	£?êùW8Ø??œDÿ1¥žÈ?–…y`šó¬?1\"w?ÁIóðcf?›í›,t"AGN4FGL J1837.0+5347?×bL£7b@7£¾ýq?À:"
xÀ<nCe°^@n]ST0@Ê:KUhè?µ'éÀè+迅Ln:Á?Í+éþ5ûe@æ åhã¿ÔŸ¯=æÜ¿èT×È©Qž¿çõšÀ[¥¿ãXˆAØg‹¿ë>"_¦XÅ¿ïÿ˒:)ÇAGNbcuNVSS J183710+534704?ï–[')Jã?†T)œge?oÕH_×äS?n"ýaéIÈ?'säA2?Åoõ''@?ïΎ£œQÛ?vŸzÇ><?Q*kjá8?^¶³Ò=Ž?tn-xÞ~?qVi''©à?ï!e¿¼1ä?ŒgiX¤ªñ?'H17?ƒ´ì»'ƒI?'È£ôñ–÷? YÛ\"?ï³ä:"V?_Ñ3(g??p–AxÚØ	?Rð®àôé?uw¡b=õH?T'¤-{Û?ïœyâˆæ?‹:‡?~^gxð?rª;r´?""ÍLƒ
?ŠÁñŽÔî?ïdv-‹Û?•ið³-?e˜œly{?t˜˜«°C?¾&ÁµÂo?'t¬ôÝf?î5éÈþX'?–= 93è?ŽS§œè?‰òדô?ã?¥ƒå
¥?'cKd^M?ï%lNîá±?{ÈÖ!¥?‰ó€×(í?sôp9¬ÔŸ?Œ±kiÒÎç?smLSAGN4FGL J1837.3+1052¿ï-ÆH	•@ '5ø	'À9ÙúàŽµÀ;±Àn¹@gýY‡…Æ@b<ççÛ?ÕvŸC§ ?ÃQ]?ÌÐ?ÿºC'œüû@9C!ór?š¾\È¿Ýà鄓x¿ê/·éùr¿âu>`bì3¿çôñ^|¿ïÿûÎBÓAGNbcuNVSS J183713+105143?ï\›É
"W?†îVýk9Û?cï4Q¨€ž?`ÌàÓEá?'î Zs¬?…[ýñv¿?í.2àIx¼?´Äö2¯|E?ucS'–y?xrO|ÎT?µ<'È{ ¶?´7ÙîÆ?íâATDa?œª§ˆð?‹Çªó
 ?‰Aޜ­ö?ªéÿüc¹?—zŽ	Å0?îAԙõd?€2
?{3Ý@ý$?V§y€ß?¨|:Ã]Ræ?~'6…1D?î²[ûåzT?—Ò¹#aSä?x–GŽ¹³—?sÂ~@UÄ?¡ÇwSl»I?•±\4Ýx?éË»ÎÍ®?Ã=a¤#¥?Êܦ?_ˆ?ŠH¢À¥?ǶÿEšéÑ?Â¥>ލ¤?ì
¢w["³?¦Fr'/A?V¨œ½
?˜d&¢×z?¸=B<Ñǧ?¡Çå¡|^?êð~Ý?™¢õ+ôL.?•=›Ø=bD?xU|ŸêìÊ?Á–T71<?˜mÏwBAGN4FGL J1837.4-1646¿è…g0ÂÀ9åâGˆUÀ9šsfÿéZÀ;úý9@.Û'X‰"@¾+Uï ?ÕOƒ3є?åAˆËëü=@R
Á‰¢¬@å?ïÞþ"v¿ÓtnÒE²'¿è<Ÿ9@>¿î¾£%¿ïÿÿ)@k*?ïøš°ðÎ4AGNbcu2MASS J18373301-1647530?ɪÆa<Ÿ²?ÚË6¹i?£}^õ_¼I?¦£ìé(Ì?è]xwú§??ÃáûזJ?ßߙs
 ?Å\:¡Í¬?¡âéêuòN? º"SôÍ?Ýä	¯¬*–?ÄpÝØã±k?Ýóx\!ò?´Jaù\\S?»Kët?¤êÚµ'É?Û9Ã"݃1?´q†¯¸é?ÛwQ–Ü·?¸¶bTÃW¬?©"Ùžð'?'G#îU?à«	›+·`?ºŠ¦Æ}Ó?Ä*éԀ±|?¾XÔé"?§›øëC?­$õ:¦°^?é"{ÙPyü?Á©'UW P?Ëy‰—?ŠAÜ]'g?°'r¯¦Êz?²R¸I '?ç:³dñÇ-?ÄÝjÇt?Ó}
5·a?±Ê"ãfù?¿H¾•@]?¤wI6ý.?âˆÁ'|D?³§MʖÅ2?ËJ骠tw?¶IT*ü7[?®v™ù/?£ÏñøÞ×?çEäËÇO?¼GVÚñí\MIXED4FGL J1838.0-5959¿çîiÞ§&À5¦¾zúr"À:®Èú°4çÀ<~PŽÌÝ@ ÀR¬u>p?ùÒk<Žüˆ?Ψ£!ؗÜ?Òw¬tg°é@ò¿-§Ù@¦žûn¿è›¤¡4˜Ž?î(ø|}ÿà?è7é{Y=¿ÖXF½ÿ}¿á\LœÄß¿åPŒ?>qAGNbll3FGL J1838.5-6006SUMSS J183806-600033?ïЩ"‰V?cÉÈbË}?HCOÅv?8V´v;úP?t¢Ö^¼èð?b3Ý>•U'?ï³R"1?"¹Ùã³.›?[Ô
æ±M?k¸Ñ5óÈ?Sçm•å?U^"û?ïQ±Ã±ðþ?…%Ôã¸ä?nõÇdÿn@?q²ôÇFÚ?'ë—¢'t?÷RH(Ž?î
áSí?‡Þõ±Wm?}Û.£M?Ø?f2TƕÍõ?ª³Éý(/?†Q5"€?ðÇ[?vÛ]ö3°'?`~AŽg¤»?U6ðžåf'?…¾sq%ü?tž'tÞ?ïa‡"?›C^yˆA?tîæú‹Ñú?"»8¤ûå?—¸%è'N?–Õ!£¢?îÄìxä˜F?'2¶¬<?v÷nž/·?v‹Û™Wû ? î'ê3?·Yyí!™?ìZ)Ý?ž¶!p°DÀ?ƒ°·:Ù?y1u‹ÏÙÖ?º¹hä<ww?Ô®ÿ˜;AGN4FGL J1838.4-6023¿Ûk]œoÄÀ5Î/ßÁœÀ;Â~•1UÀ<™7¨ùä@!aéÆ,ʎ?ý¹Y_ç?ǐÈû"?–†¾(LØÔ?Ñcº¥@·ä$\V?ïå$|·
Ä¿ä¤ßßÏ^¿åOV_2?˜¿ÖE@[º»Ó¿æêNˆ#O¿·ø'wAGNbll2MASS J18382063-6025224?ïëúÙ
Ùß?WK3ú{?!g÷×å{ï?e±OÔ$.?bî§2Ìjƒ?VqN`.¶?ï²õ48ۃ?€e@@N?S"é†>ç?\j¤¤'®‡?€ÞÀQ€±"?|ö—9¦Ã?ï5H¥úë?€û>?PxîÕ;€g?7ä´ÏÙlã?£óšÅR?€ëNÑÌ÷L?ïbs)î;?vBÍÁ$´&?T»ûLÝ>?;ŠöÙI!?'eáæw^T?vLcèÖg?ïÓ¬P3´?l‹È¯^a?25%Åàƒ?$ºÍrñX'?u…¢Ž,K?kèólq^ç?ïMé
?–'4°…‹?[Ÿ5:L?fr$ãIÈï?"'*½Ì\m?•tøVf´­?ï¬A«µÀ?*€Èl‰Ï?Ud¥f3b?H!х¸do?œ´-i{¶Þ?Œñ±Sa¶Z?íÚü×<Îy?—™^xjÒ?o¤O±•M?`9&9í?°/""]#Ò?—©5{´l´AGN4FGL J1838.8+4802?"|My°í@5҉üm¤HÀ8Y…O_¹¤À;'*è´@¿õ=Ú+/?ü9"ù÷¨?¡Dª©â< ?§Í?¹Ss@¢ÁE°
y@#3d1¿ÓbÛ, Å¿Õà¢A³Õ¿à-n}ŒÙ¿ÔhrÛâ`¿à¡u0.¿ÚÍÒ»ú²AGNbll3FGL J1838.8+4802GB6 J1838+4802?ïö£—x$?AK ¥y¡¾?!0È}b?³+ԕd?P"ËäAuþ?@)£zә?ïã
¥0·¿?jî*' :?@eæmÌ?J`hè¥/?hÛáP´Ð?f¡šÅ?Ç
?ï¦ïVÿ/?{ý…¸p{?X.©òfi2?^g:0¢?ƒ>TüÀB?zï€5s?ïæù"v·9?Lœsvâ?%soSb/?Šÿš$?g­•*›Hi?K=‹Ïø±?ïîð£
-2?T휹©@k?'بÖ?"?=cƒ†¼?_#¤éd£:?Sç*5N'—?ï©-™Ò_Å?‹^"ôAs?SrÛcñE˜?a+Ày2–?ƒF>+H}ÿ?‰ÖDÇd•ò?ï•Z0Fð?"~aá¼ö?Y¬{òch?b!kH`B?‡sèÁ0G­?ƒKÖRá:?ïÏý]Æ?cgkµ·Ý©?4žÿ*òË_?#âI"ïF?v·'ü\Ñú?bñ"]ŽxÄAGN4FGL J1838.9-3457¿Ñ¬®·qÀ)—¬>·Ë´À:NÒàD²À<DÀ:î˜@#ݤ
‹Ê@®È b?Ä	çƒÝ?ßa¯²à'|@Ž6Kìg@ðÜvü?ïø©"¹`?»-(­Z¿áÌHþv"¿çà,€f—º¿ï¦tÞÏ-пï­ðÔ+AGNbcuAT20G J183923-345348?߅ë5‡e(?Ä\EяM?Öø¾M<E?ĎÙ%um?ìúì½%?¹¬~§þ?⃺XÅ­¸?Ë:œS]J3?Ó\:àâÀ?ÈÁÕŒUc?¾qØNO>?ºšÊy¾æc?à@³º4Í?µˆ=ž€?ÕYS!©â¬?´'ø¹B^þ?ÄMíÃgs?ªÔn©A\‹?åƽKÿ‡? DɈŸ¡F?É+›>{?ÒaûâRà?¿rߒï}É?'ê;,,×ð?ÐzçRñ$×?½éa` ²E?áÃ))Œ?Ãö‰ÖûFT?Çý‹]¹$?¹€TQ¥‰ô?ØöŽaØF?ÉJwÔwç?݃‹_3?Ì#–ÑíË?ÃÙ;^ê‹?ÀD–À˜®?Ô )ûøy?²æ:1)BÄ?ޝ§Ô"Š!?·ÓÂÎ=³?Ʉ\aúË?°»'lK?؈‹59?¨ÜÌJü¡?ØYýŒÞ[?­·Çß«‹Y?Î:î{Ñ»'?£ëÄ)}6MIXED4FGL J1839.6-7107¿ïŽ¾Oœ.À8ŸØ­«ŸVÀ:ƒñ'¨4À<l'ÐR@&ò	GQx@a<á1ޟ?Â6‡»öÁ?Ño^|âÿ"@ƒ)›üå@J肊ßB?Ð%óD/Ú¹¿æ*#ŸÂR ¿ê܍YýL¿ì\e'TPº¿ð?ïÿÖ°cAGNfsrqPKS 1831-711?ïåló73?vüÓ½dI‹?XàOIú?iŠLì5&Œ?\EÊ£Ëv^?oUßDót?ï®wŸÀ?"a ¢ê«?_Ë:È@Ý?i>Îm'?€hÒ®ækZ?wƒØYÎI?î¸Å…t_?–J\‰í?Ž™{©©
(?ŽzÌù
4«?™š'uº•ˆ?6	]i,?ïÊ£Îb	q?^ù96n?O'_L—>E?6çtœ}?v»ìÞòµ†?\Hï³ÈÓ?ïÜS݆X?t/&Tñ¨ˆ?_öã"ƒö`?khðï•É[?c±qn۔Œ?h»÷…º¾?ïÂâ¤`®? —v½Iº?tbsêìÉ?‡¥êXûy?—o´TNï?™ùÒ/}Î?îtè_Oq?žFQëQ"•?–JA†vì?"°¨U©h?£(ŒXkæ~?"N;ø(Æ?ï+n|í€?'ƒ‹õú?p$ÏV^?^Ò!Çç9ÿ?–‰	i$?€×¶0cU&AGN4FGL J1840.6-5545?êÌÙYøïÀÀ4²ôàM/À:"µÄr‹8À<95>»@N©•·b@i¦Âwu?ÌF³Ã'dÂ?Îå=F‡xÛ?þ{ƒ@GþЪýÅ¿¡1=ßoοÚ]7þôè¿êßß~€8 ¿à‰T!ÀD(¿ïþ_–}Û?ïÓä^
ýDAGNbcuPMN J1841-5544?ïø98ʐ¡?AwDSBÒu?8´¨ÅË.?2æ¥.ÀqÙ?BÀǍ˜[±?6Üy<Ä%S?ïêûVö©?ké\ úìÝ?6¶gº›ÐÈ?N'JokµW?b.¦*_ô?fîîo'¿ ?ïkÄq‰…$?"ú9žð?rä¤ltà	?vä¹{[?‹œ'kƒÎÛ?4ù¸¼jA?ïø&3_AÉ?6¯e°ç·û?±\…í6"?·i'±C?LÑ—í}¸?5ˆ¬È@IÐ?ïõ½>íÚ?IÙVS‰?>#âsC²3?5Hƒ¡Ô?IùžrIð?D.¿ރÔ?ïì/À?ƒ¨;+zÜ-?L"‹næ ç?h³'±£q¤?z—mp£?€ê8'À!?îý !є?'lî‰Ãµ7?~G\Óp ?åâ 9.?˜º$"-$î?Œþ¦Ý¦™?ïåL©ß?Zâóì?1"g—#9Q?&U²+ñB?h	ª	7?Xè(}Œš›AGN4FGL J1841.0+6115¿ï¾¯¸"Ü@8ÉzÝð,À:+ª¨µ–À<"˜8p‰Ö@­Z—@iøÂ!?¶e Ÿa¿"HóÜ'«?Üùm'e™@šš?íˆZ吿çs×¾}J¿ë%§>Ê¿Òft©H›¿ê|•aütZ¿é‰@»±òVAGNbcu3FGL J1840.5+611687GB 184000.4+611120?ïïgÈ«?S(M7c?DóMy7?8ýò—,(?WhXàÀp?MȒ1ûjl?ïáËד-?o!²|Äî??ìÃ~[^?JÍc€~?j7`ꨌE?j'¹iƒRa?ï(B"O?"Iù1¨nG?jQM²àÇf?sX·ÿn¶E?‰)¢ˆ"T?=Û4P?ïÚ
#mÝ?Q¡ˆçŸÕ×?LED÷%T?3onáà'?ná‹jÝV?OҜ^¥(:?ïàaÌù˜]?d-|ì`û?Uj}FÇ?K'P'a°ó?dèôu[?w?^Ð'£ô˜™?2?‹PWÃØ?Pj=hoÅÖ?[VQ8¶c­?†n&pÅ?Š)áÕç`s?ï.µüëg[?‰ÿ½íô?r/¤ÐßÌô?u
»‹­?•W'ÿÚ^?†ô§aLY?ï€ïe(#?tµÉ¸‰¶…?ms>MJ?^Ñ»:Px[?ˆœô…J?qV¦v•XAGN4FGL J1841.3+2909¿Óg°Òµù@-±«ŸU›=À:Vî#^ªÀ<)Æ°Sƒ@!ÏYè~¯?ùP¬:†
Ì?Äd?D¹mt?ÃÄ©Ü¡V@nÊhn~c@ØíÙ6èt?îæ{_ïJ¿è±Š¼‡l¿Õ"!'—ô~¿Ó«é]&KÄ¿ÁƒZèÙÉ¿ãúM~caAGNbll3FGL J1841.2+2910MG3 J184126+2910?êFVä=VÎ?Æ[
GE~?s]O;¾{?jäiœé®?ÆK·ƒº_7?ÆgÈñËß½?íÜW¾Ð,J?²ˆGD‰³"?¸›'G?'Uì'X;d?­ùÕëð®?±žvðn´á?î³4Üg?›Mç4D?w!¸ñÕn'?uÈh9ÔOâ?«ÙͲÃÈ?š|*P"»?ëFRZüâ?˜-°Ð2?ˆóüËÁU?plôš#0Ì?Â/®—5Câ?—dYÁžb°?èÙ~®S1?Çñß—0ç?ŠTå©uVZ?'ff`çn?ÎKªxd?Çü,gÌ?ê÷;'jÊq?•ùoÑ	?–ìãÈ°Á%?¢¹S©bsï?ÁEvèÐʙ?Á6Ti¨~þ?뷚"
:?¦Ò¡§Hó~?‡Átµüª?"b²ýÖ?¿JüÊãµê?¦,^ÅžI?ãÔA6ðÆÁ?­Ý®[Š?™tà¹za?‰ûÅïÊ?ÖÀ/'NW¸?­ ò·¾SAGN4FGL J1841.8+3218?ËwÑþdõM@/ô(²¦°ÙÀ:&jö±À<'-Z¬@ h–=º6?øå'Á(?È-Š½2Ðã?ϓºÝa @ËýÝï@
¹é¹S?ï×O!¦Bõ¿ ´T0ý¿â4»ÉoJ;¿£\|$56¿ÙÕÁ½ú÷Ø¿êÒ]«AGNbll3FGL J1841.7+3218RX J1841.7+3218?ïÝäšøä?eÉÕ¹<ó?KBÖåÌ'?E_PÚ;ÐH?kJ°]€?bµ½ÖS£?ïÔùÀå|¶?w™Ïf"1?H*"ãS?S³¹úcé?r}Ü¡AˆÕ?t¡m8=ºE?îO«™ì?šË6¯ˆ?ƒPNç	µ?";e2<Ü?¦?;rO†Y?˜îôêΠ?ï1µ¢®Á?tÏú½ïŽí?b,ÅÉãåH?Hƒ{ô~A;?—ƒÄk
'=?tûQÒ?ï´Ø³?}Ðb›è¾?[®WV'"ß?YË-ýŸ–ž?~¨b6ºQú?yx•ú½ö?ïtÂÞr¢Æ?•FG'S5?aùʟ‰'L?qüð¡SO?ŽPÕ°v)þ?"wO+‡#?ìÕ	Qõû?£Þðž–F?"u¤"ÝÆ1?Ž|GiÅV?´zLnL÷›?¢‹Ônˆ?íù.2*0?'8{ò\Ž?sL:µmh™?dϞ¦XJÃ?®˜YáDi?'Òö5§AGN4FGL J1842.3+6810¿Ú&É "'Û@9à(=5ëtÀ:5óÚó×À<FõÉEXÐ@"ø4.°Ã@.d"Õ?¾§à?†d?³?ÐÿŒh?ñ{½•ø$i@ëóbål?å}>" 
Q¿à²ù¢í]¿çýªðÙòO¿çV²X­@¿åÿ~?ËòÝ¿ïý:ˆ'
YAGNfsrq3FGL J1842.8+6810S4 1842+68?ïÜ÷ü¾"?lÄm¯?Né|55H ?Jj¾ÍÕó?kN¨Ôö?fÍÞ7åB?ïÈgXºèZ?sü-ª^–?TèÙrD?Y‰»ž²Î?vÈYqªg?o4sb?啕Ëù‰?xpà7á?ZÐß8aï?]FlYp7ä?'7qN«m"?v˜Ô'º¹1?ï
Å̎ ?c´=´ir@?s]Qª·}?P9ùR®?†å¸)rW?a˜ñžSjÉ?ï£6]V"¯?ƒk·,«Ep?d^Ã(
"?`ú ícVÐ?'·ãoõ0?€%	ätË?ïlêLmš?‰8L|?`m4Ëд?dâ[Ù]g"?UíW®?†¤­'ZÇ?ïMæÌÁÿ?‡ðiëô2×?f¯r¼e—y?^Xº&èH?"xTɇ¨=?†Ï釤–Ñ?îe$Ô9—j?'äZ²¦úa? æ™@r%?qgSž%+?¡?oÆPK?€=K£äšAGN4FGL J1842.4-5840¿æY—$c%ƒÀ5Í!…Æ~À:'FÙÙ$ÊÀ<kÕW2@!ßX6øº'?ùµ>U¦$Â?À¹e¼ÈGØ?³ÒÈ ~vd?õÂäßJ@c?cÃ÷¿ïv³…Óé÷?î϶¡'6y?¥'@"ɝ\¿Òëý?Ò¿à±6¤û©¿ÇNògHºAGNbll3FGL J1842.3-58411RXS J184230.6-584202?ïê.ÁxI­?†ê—çQƒ?¹T"Ì‹/?§ñx-/?eséåîþ?†ds?ïì!øX?ghY³`!?+YT'hS?<Æ°ˆÅ×?b7Ùàˆ?d¢1þ]É?ï;´†¯Üý?š]ïy?Jõo¼Fu?6õ'Ø㻺?—±ÆÍÆb?¥Yè¿÷›?ï²ÒiˆžŽ?aï¸âŔ˜?AÝÅ×JMž?(ß¾sT?'-‰<âƒø?a©ë¡¦9Ú?ïð.Lƛ?\™KSXB?(†Ñîä ?$m¶/dï?\'Œ–p)<?[CXËmY#?ïÃg"€~?'Z²D]—~?>݄Þv?MùìEºu?|^]©äuw?8oo½ê¿?î·=àFi?˜{~Œ´*?PÂýeHh?KQ|ºv."?¤bºª?˜mûè
™K?ïBpô'Ø?}-QéÌøÅ?Q çôdÎ?>øuúºA÷?–ŸÒÿÒï¸?|ëÏg=AGN4FGL J1842.4+7613?éŠ*M'ó[@:ўùTëÀ:þ•{&çËÀ<zŒç¯¸@ߖK±YT@õ"yŸ(O?ųoC.ÓÓ¿±pþöÌ%?ꖝ^Ë@ÐÕ¹ÛX?âTO­¿ç`|wIãy¿èHèÜÍËпæ¸þ˜¡Í¿ÖÎ9Ì¿ïúµ¾=gêAGNbcuNVSS J184225+761046?ïß¡#·ÑN?' Nˆ†ô<?W9%WQ?}*ììÀ›±?dÑ¿˜aVK?‡(/ÕøÈé?ïƤò"/ó?‰ªÅå½?V&q-êžð?rŽÈ­ÊÓI?w#êvœ
­?€š#
PÐÐ?ï`³Ÿ‡ÍÈ?'UF‹±Ü?d_eçÙ?j±ßñ¢±$?']«qýS?)êwìx?ïäxZq?P/šíMä?@òCKô?/tƒ[ÂGv?gJî¹ý)p?Lìæi
³æ?ïá^™H;?m$ˆ×ɺÓ?\×öÇS-}?\ê‰¹åÕ?`5åâîm?eᎫŸ-?ï'è7êۉ?YîÞsí?^Eû[w:?r\
€qÙ?‹}2¢íêÏ?ŠÔ|¨ùÝ?îÂ)žñ? <:·Ä¤?r"ûqa'?qÿÓ-é?¡Šô7ψ?Ž|é8'	?ï ¶œߣ?qõiF;2ç?_ýÀ½ï‡?VÚpzJ¤?ƒÒ¡µV?on*Ëõ¨3AGN4FGL J1843.4-4835¿®ÜdÍ¢KÀ2Ág#$È6À;#jJ µ'À<"Þ·°ÛÕ@ /(Œ't?ÿŠ"¢Óä?ÌGOŸÐjf?²ÐË_ƒQ?꤫`kz¢?ù!¥AB•?î"þ×áÓÅ?ï™G™ò"í¿Ô'd=AT¿éÈ»ÆKç?ÊSk¢ep¿ðAGNrdgPKS 1839-48?HsG‡?‰šÌä8"?E¸šxŠÏ?BÉDÁHßÁ?ˆ€dEM1Ï?‰FÏÞE¾?ï™X,֑‹?ˆä]¬¬?a›çŽ"f¦?kéÂ#ð?…Búéz3v?…wR²¿a?îâ–Do?¥'o_¦‡?q%ö—Ë?r×HáÑ-?Ÿf-ý€µ?Žn£íÈ?î¸Â-%kä?…Þ,7ïÅ?k‰35-©œ?am7x?¢»IöüÈ©?"œBÿ¾n?ï©OD5å?Ÿý‰oâ?ZÂ]Þ±"v?XÃ7Kh'¤?›~°>‰™?Ÿ†â?ˆû?îÿA.çÓ? µž†3"|?uQiS_?eG›@?šÃuÏÔ­Ü?œ1ÉXÞ?î5-ß6[Ý?—. #áÜ~?zg#äz?{Nýléj?©`=©(?•A?ݲðz?썇ú­'7?¢xgêŒÑ?}"´ýØj?wÙb\.n?¹ºtÛt/}?¢°ØœÜAGN4FGL J1843.8-2011?¿:Ë`™¦ÀЃn—À:§\ŠD'À<\W=Ôvå@Þ^eþj@Ðg¤T?ÎÁ#vQÁ?â":Re@ÚÙºñØö@ÑË«`?ïÿ΁ز´¿È=䧉ò2¿´l¶!9¶…¿á[ā¤°N¿îɟ†B¤À¿ïôÒÛÇ5AGNbcuNVSS J184339-200606?Ù@m͹Ô?ÁÛGP˜ì? 8D?%?µpá3tC?ݯvÇÿÕÛ?ÂfŸø"Œü?Ý2ØmG‰µ?ÆýÁ
žE?·4勛»C?²L·c†?Üÿî/чz?ÅX €´ã?åÇc²4£©?²~z.oT!?Å5 ·'–?¬{÷ôRT?íQ1uîÅ?¦«!Îgõ?èz,·/¢?›Aƒí?»y=·#K?".•&³Â?À''îW?"D'Núí?ÍNbE'Ññ?»5™Ýê´ó?Å6Āö?»?Jœö	K?ã^ß½{‡F?…bï¨2Ó?Ð÷iíÉ5'?ō/]»œú?Á°ƚóP?¾,Jƒ(`?ãFWþÊ?Èf#FÆ?Ý
ìmb?¹Zað©Ù?Ò!úÆÛD?·êý'£œ?ÐÐè(%–›?°&Pç.?àöô ü9w?ªNÉ1yÚ?Èèí°®D]?§ÐÖ !wc?ѝŸå°jä?¦…åsìô¦MIXED4FGL J1844.4+1547¿æhn ‰@!DqæÍ)À8¢Ž`€sXÀ;[vý^ù@ó%~¿£™?ÿªúêí?ªÿö3á?¸¼¨½Mþ¼@/½jY:.@£‰Ê™–¿?ïæ(S`'¿âzŒŽ\¿Ù8i}òõ¿Ýx6zæP¿äXÅÉ£M¿âØ€_5ðAGNbll3FGL J1844.3+1547NVSS J184425+154646?ï³¥Áƍ?wíˊ®u?K[¤}ïh?Eçèíäj?dùä8øe?ua¸`óÞ?îè‹-´ÝÝ?¨2Çç*‰%?^š^¬Xò?jékå¾x? 'z,¹¬?§¶ÓÈ0ß0?ïÉÉÚv{?yL>"\»?q$_8àÅ?xT€¤ñã?˜¯N£k?‹q÷†FÇ?íèXçµ?† ŽCcÒÄ?xVÉ›f?Vú،À5™?®sñQWÊ?…n›]!?ïY2«ùÃ{?ŠÁÏos¾.?T§|ÕïXc?Pÿ"଴ô?"2ª¥š)?‰m7'¹Õ?퇭ߴ?·›v†²?r#»¨²C?‹Lű(€?²¤ÐÃøü?¶ä-i—3¾?î˜$.æûÖ?–®¼±ðª?xѧ·Ècq?¾R¦`?£cˆEyº?"³jêÐ0?êÚ!^B? Î+ö®U?sbH*®X?p×¢¬Ó^=?ÂÀDdo&? 'kâsŸAGN4FGL J1844.8-3248¿éõô–WÀ*)#å¸VÀ:ßT¦Ë±À<VÛÉ¿Ò@ çk $|?ýƒqÚ7ï[?ÌBûRFI?ÁJ¬ ¯Íã?÷<c'í"Ó@¸c3V?ÝØ̵O؅?Ù›ÍÀ"?ï&;Óë¤ÿ¿ÔÐ{)Ðß¿ÜöØ9™…¿ç>¢ÉAGNbcuNVSS J184445-324641?ï°äÎ:$?qFùSˆ|2?C³"ëgŠ?4;_}Ï?'‹"+tW«?p¹¿»¬'ê?ï‹ß¥ÓŸá?š+Õ\Y€?[Ü$îÝô?fæv|–!?‰Œ'æuT?™T°¡ìû÷?ï\Þ({"?(Ôê§ ?a8Ötç½?W">»Æwñ?'= ·?}¾™üå÷?íS³u&·?˜¦R€#¨†?|•†g <?k¥Ú>€;u?¶ù=G?—ÊùL­cÃ?ï_Íw'æ?'´GÿÛ÷?[¸¯H×Y?P&÷Ty˜·?'jºÆÖaÎ?Ûs²Âóû?îË)aÖ½D?©|þÚv?kƒÕÚ_?{žÌÑÂÂ?¡›¹×Ã?§ÆӛjvŽ?î—YÅ»'ð?'Ë1Ä2?mö¿lÃsò?iÂ/±é²?¤ª÷®ÛqÂ?';œýÏ?éªjۍ|?°2­V߆?ˆß}ûgŽ?†;n}ýõ?ÇÊ''?X?¯¨Æ$•uCAGN4FGL J1844.9+5709?ÔþD]@ç–@7`ÿ—$tTÀ9æèˆêõ­À<pOŠL@ŸÍ¾G[@h§¤WÚ?´Jßø"»í?¦³À¿Ö͵?ñ"wXüñX?û`gô°ì¿æX¨mqób¿ÜÀff²g¿äiÿöÅÅ¿à⣘öÜk¿ãö"¡¸!¿èÖNUÎAGNbll3FGL J1844.1+5709TXS 1843+571?ﱍ"†<ù?r14ɶ¹?V7{™_×;?LÀ)2V?€Õ«[v'ë?oŠ?Iòy?ï9qȑ¡?'•‡Iš~?| éoé5?€BP‡M?'©ŒM"Ò?‹¬NG)Ã?ï#-s–ï?‡Q,µ™2?xí«€¶?v£·Aõ?••Ö*>xÿ?ƒ~ÙR­Ô?î†lE£x@?€DºÖ"g¬?–…—¨)Š?tµÍÙ]í?™ñ·Xj|?tøYi½Ò?ïKë2éaX?ƒ_Äà"Ò?k'÷˓f?YöÓS  Q?" 'f!?ˆØBUÝ?ív€B?²ñÂ?˜.ô;$?¤ê"îð?¬‡ýÞê;?§Ûl1]n?îsšÔ­ø?"€.qT?'t¥‰ˆõ?z˜õ"yë_?¤))P"°™?¢•ahµ'?ì-mAÞ?œ-á^ˆ?­¿PC?'aƒDñá)?°6J8	;?'Býa²PAGN4FGL J1845.0+1613¿íúš<§:@!cåÙä"À9Ñ°C)J|À;‰ôRLÓî@+³Ö0Ϊ@ïsÚZT?Àñ®X˜r}?§;ýå§?é^«QR+@ç;2±A¿ïü+ഐ?ïû4SÄ£3¿èe­¤™`¿åøç¨eݿᆌáû2;¿â‡¹1åUZAGNbcu87GB 184225.9+161105?ç½+w°™?¾Fc‰Ê ?wy‰éD?hŠ0æ<ãs?ÑnŸ"Ym?¾7Ë°ý?ìÆ)F©€?´Q¾'‡GK?~6ÂBZó?‰-
ž0ÿ"?·î\P¸Õ?³v¾ôk#?çÏJ*œ?±yºu'=?œ.«@yc?Ž ÕZâe?Ð:é­O¦S?°¹ˆ>=Ør?ëá8J…p?•ñä—?!k¿?o…0¤B¥?½SÔ0¡æù?"ÑaèðrX?àKè1y—?Ä8I/ýQX?''rl¡Am?‹vËòþ?ÞA³	"bÚ?ÄKà.ºŽÃ?èÉÜÑì`*?ÇG*÷O'I?'WŸ¯P2?™bߍ©±?Ê­˜Ôø•S?ƙœÃ3Š¶?ߌ2&/?´±<ïy¾ì?«/®np?˜© ›È?Ýx• ?´þp—‡ñ?æ|må¥{?§l(»=¶Í?¡n~Cø‰?‰ŒhU?QÃ?ÐÙôP¹?¦Û‹\cŸAGN4FGL J1846.7+7238¿ï ¾#Å5@:%9C¬ÅÀ;r«¯EÓIÀ<õøٛi@!‡Ý^?{k?ó|tðlå?ßÀç,¬0?َޖxÓ?ÿ›x¦@ÿm[M-°?í[Ý¡[Z¿îñÄhz<Ý¿Ñç3À̹W?Ú¶ÁÚUv¿Î0¥å,j¿åÐîš|îhAGNbcuRX J1846.1+7237?ï½*öJ?{C¬üš"D?ST <2Lº?QËIaÂ@˜?|•ËD;¸ ?x-†f-%é?ïÊd÷"[?}áöÚ]·?Lã Afùý?]–Iöë?w1Dq^"?wŠ+BG?îÂ-fb?•B´Ê;g?q·Ærƒ?x~°>á?¡¹2 ˜Ë?"*~'Â÷?ﮝ¸?Ռ?h">ߎna?5Ԉ|Fo~?(Lpeª"?ƒ©í¡D
?h_rÍñÀ?ï†ì'Ý4E?‰,ª¯ Ôè?`×o(ÞñÀ?]ƒFø>b?Šÿ†ºB&?‡<³Uu?ï|‰­µ§º?}O;E‰?Wma"¸·›?j_p̛w‰?ïèc^Ò§?¨Ý½œ?í—e<ÎE&?¡fíH8?q|<n̕?zt•9ÚC?²-RîŠ? ¼mÀ3ž?ï*‹aD?‡ÁWÀö?A)iíˆ3?C&&(óú­?œRV76{?‡´>"¡ÅAGN4FGL J1847.6+5219?ï¿T•>Ò4@5¶–6—lÀ:ñXeò£ À<¾ÿ
6º§@ljßgY+?ÿ̀CRe?Ðc"GÁ`?Ð	ZÝN@XCùTT@z$'±rÿ?ÛT9}¥Z¿á*¥Å÷Æv¿â&©ý¿ÞÓ¿àÐ×ôH;Ù¿é¦n£KÊ¿ïÿþÞ÷AGNbcuNVSS J184754+521513?￐ª˜ÖŒ?q¼#æã#?hÀåÙ#Jo?`x0qA ±?s×7½d,®?gúâÒý!V?ï«Õ7îÉ?{š>ÿ?a"/¯°V?eLÓÉel?€©®@ðã?tÝ=7úˆ?ï>³&?…dø
~?tR\Rk#¼?s8óóÌzË?"
vß^R?'úî>½?ïV"¢¤Ò?jú¡'M'?{‡ùéýhƒ?V/'#·u?Œ—;pn}?fèœDò]ã?ïTD­Ùír?‡eë5ã«?*…>Š«?sTƒ	"9B?‹Y'úew®?+mØOÖ»?ï?OBªÂ?"ñF6—­?uêó£ƒ+ß?x…ÿ?˜=Y11–Ê?ê÷X‡B¹?î}¦m
"?'ÐJÊmeÎ?†¥–DS?'¾Vô€?¢ ›ð¥³È?ŽŠ›íy?îZrÛÐÜã?"²TYÖ,?Šô·Ô@9?rwüë=p7?£›¤KN]?'³È'Ï7mAGN4FGL J1848.1-4230¿¯Öâ«TƒÅÀ1_󾩛À:Sˆs©À<(ôB\›â@Ä:P]æe@‡zÛ?¿e')]œh?«$|a$ˆ ?îVužèŽ@ø`ÍöŸ?ïöðÂuZö?ÓÒ)-ó»¿é¡¿ØȄ¿á|×­O¿æEòèn¿ÕÏ°¬AGNbcu3FGL J1848.1-4230PMN J1848-4230?ï}TW×=¥?'S0ӁL¿?hûbƒ :?rR846ß?ŠlXêhC?|#@eñM?ïL_1ÇV?€0—kyÈ.?aÄ´b?`­³ðCˆ?";»'?}NªÜÛS?îð5d2Q?Ž"¾Œ™á%?{›"Ky3ž?{°™±¨?›•ú?‰R	¹Çtd?îwâº^3?xö-ìfãì?ˆ8æ'(?dÀq"Ý‹ë?¢sÌdùÓ?uÄýhÃ?îÔ@(äû˜?'OÛ ÕA?~,[|ú9?wX¼š¨Ÿà?öoËyl|?…ÆzO4?ïJê"âÈ?—ù©¹G@?uÍUÑ H™?†ÞHÜý?š#M?¬pê?"Ñ/Ä$ó?í¦3¯Z˜?O&²k'?ŒÝ"ã_?†QXÌÅ¢?®eiL…û¾?˜€Mi֍Š?ëÁd+x©µ?'rŸÒNI?¡£kã$"b?"T¶-¡?¹#(²:u(?Žñ"./83AGN4FGL J1848.4+3217?æCò{»•Ë@-_r'Ä"BÀ8'ÞѲÛÀ;il«$@#åÓ©‹@B[úҙ•?®(~îÙ£?Ç5Z«'@ó<£~@ŠÂ'4›¿ã'—|ˆç›¿Ùl`üD3·¿â¤«ã¢Ò¿ç皮l¿èʾ­	c¿ðAGNFSRQ3FGL J1848.4+3216B2 1846+32A?îVŽ¸Ñ(?®t}­å1ò?£¯ÆLm%?˜!_Lþ?£.(}ê¿ç?©‡Dµ3?ïÒé'Dw?yî)Ώ?MÕЉ…äè?`Ãâ|õ?rлƒtT?uá´<"z0?ëT²w""«?ª~˜šÏæ?±{6ÀRã?¢@~¿0~Ž?³ßW¿ É?¡¬j…¨ú?ïxU"\?r´³¡8¼?R
&Uœm?=³ï	ÙÛ?©V
e~?qÆó'5ÕE?캌ûÊ;?µc+㏅9?¥+B¥¡M?¦~¤˜¹A?¯:?Uˆü?±aƒi?ïzNr PO?•Ï
¹-?bìZ‰ŒQ?së4þ¤µ%?Œ±Lîº7?"Æ'pìg?ê&͹~2Ø?®;ô&FÕk?¸ì~­íÔþ?§1Ú
Ö{U?µÝ…² À?¢Ý£t1»?î‡,šî?¾‰yL-f?k\Ü5ඈ?[ú'/?¥ÚMó;?q쭏[AGN4FGL J1848.5+6537¿²ªÖ©€¨˜@8Õã§Ú¤ýÀ;1CºióºÀ<Ú!›[:¹@!'³­Áð?øçKƒŒ?Î2Sº<Qj?ÆÈdȬ©?ûõÓ £äv@ö{¬ô•>¿çW>«6z¿í²1«s¶±¿Ì"Æv)¿Á!JÓbé¿Üà4óý">¿Áº†ú¾VAGNbllNVSS J184822+653702?ïÕkõq‡?|WƒTŸÉ?=R¹{ÛDi?:Qé§ËeO?s¨žŽ…È6?{]‡î?ïÓn*fA9?rߗ—J°?D¶g¼ñó+?PLÔ{ÜTU?s²à?å+?p\ÏîN)"?ïyV5ÊE?'`…Ü
rï?Tk }/ í?\ïãÒÆþ?›j7úÿK?'p÷¨²U?ïµ\ÍOBw?aËR/Áô`?A
%l`?'þBlÐÀí?˜*jJO?a%
j­ï?ï¦Ì5UÕÓ?‰)—7›v?NUýYÝ?QZHz´þW?"dR͊"?‡§Æ]:üR?ïÊâÛ¤?‡‡Ä<×ã?Sr(]ŒŽ?^‡p´_xú?Ÿí))=?†<&×D
?îAZ¨9'é?ž¹¨oÚµ?[^œ '0Â?bcDVÉÌ?«`˜Œ¢g?ž%¨?«Ü?ï	Ü"]Ö~?ÞOӓ?¬?S­òŽÎÆ?Er›TŒ)?‰œ‡›Ñh?´Ò{~£¹AGN4FGL J1848.5+3243?íÍíc¿'@-¦¥.ùÏÀ8oSö!YíÀ;®»iÎ@hé‡B©ô@ß=?%°?¨iäöd?º˜»Î!á|@`ÔV.@¨ê×ÿ?ÝN;Í5¨¿ã9€hÆ¿æ‡Íôêù¿å';C¢ìÿ¿èÐÀ⳾߿ïþ¶ôô3CAGNfsrq2FGL J1848.6+3241B2 1846+32B?ï~Þsy†?™ÍðâvoX?aÙ&àj?\dCÓê<?Œ>×RÎ?™`˜‡zý?ïØI4HÔR?rÞ«É&b?Iótcfœ?X£¶Uu~?pœ÷4èߏ?oþ-–¨?îh•S†?	áyXæ´?ŽŽú}`Þ$?b†D?¡Òì/?h?—¡ï_'
™?¶Qz
?pbüÞê/?YQ¬|¡Ó?B~d6}?‰ìÚg{K?nU*ZÓ?ï4µ
µÃ?šOOªsg?kzïLÿ?fÐp(ݞ?–+yÞñÆ?™ióDÍèÀ?ïŽû¶Íº'?"{[]LK?dªÇî±n?€;çm}(?‡`EŽJH?ˆÓAÖÆ!?íÅuâ|¯?¢¡à¥?•¥Éšì"Ž?"‰7'6¦?¨Ü£ÔaêÌ?
KÔ%÷?&±g
?ŽH`})‡Ÿ?wx¦o>öç?f±+¦âÛj?£Ö(èÖ?ŒªÝ£Y—éAGN4FGL J1848.6-2711¿ÎRì3MÀ&é§~^ª°À9éà¸<À;¹á`x@_ß4ÿ@S{š«'?ÊÀ	šÞ?ÓÈ5Ä+m@OÀ1³×@ÂMò§'¿Ì"ö%j¿â¼è‹+B¿è±`Ëò¥¿êétšпïþظ"Yä¿î…§ß­z!AGNbcuPMN J1848-2718?ëщIŒ³O?¶n¶lŠ®?'€JËÒ½,?ŽÖ"m"¢?¼Ó¢ÿÉÏA?µ.€0ÿá©?éHzgF­†?ĺ±'ùÉ?ŸLçñ2¶?ž±ø>	?Æôydæ?ÃÕe€@
?éÓÍk7\?ª[aw[…?¦SH_;æ?•CŠN"?Ãù¡¨B?¦ãšlúI?êÊÊUN;?–ï"«€èA?£­ü]KD(?}[ößdä?¿ØûùƑ?"L€bñ#à?è)‰$<±r?Á±2Oæû«?¡Ör}³Ð?˜œƒâÈï?ÊäVÒÛÀÂ?ÀÞdë£7ä?ãê1±	«?ÍðÚëjéû?³^æS"NB?³âú΢@Û?ÓSä7fby?̃º
œ:?ãԜŠâ?´¬²^¹(=?¶ª™uµÎ? «â"±¾¯?Ò¬…Mԗ?²MŠÛþ¨?äf^9#ë ?ªw¿'¤?µ
tƒpÉ}?–­
zùÄ?ÑïælÛö`?¨ úðxWèAGN4FGL J1848.9+4247¿ïÿ¤cÞ2@2wiDg8À:"~ù˜À<…uôxãA@ 2N@CRë__?ºÜdÅQƒU¿{^^ÞßS?½õc|@ê#sw›î¿ï꽟ˆF?ïÿ–þߙƒ¿à&D7guZ¿â0"!'÷¿¿Ü6^`Þg)¿ÔÄʟËãAGNbll3FGL J1848.9+4247RGB J1848+427?辰ÆÈ7"?ƒG_.sŽÎ?V7¸L8òù?O9mn?‰]?ƒÌ—8¼m-?'w	5+°†?ïݒ^ß*ë?vFhœ…?B=äi¹ÆT?PqËÙ¹˜ˆ?mÞ(öîÉ?sîS->?ïËndÂ?'"ìüކŠ?n*"ò›N?z™±Mߖ²?›ÁA–\Õ?Ӟ°×?﬷¥bŠ?`>Á&vB?[À{ß3Œ?@d´;aä?Z30õ?`ANµ2çà?ïX÷æ+±??#­Â?hMóÙü9?fÿ4"¹``?'×D»iú¥?Ž\HQé±Ô?ï"ÏuH¬l?‰f_ãóã?Uñ»N:€?bq³~ΎW?ˆ
ë6U·?†‹;9þ?îLˆA¶s?™èlsBXD?iÞæ5™¶ë?o™ØÅZ½é?©™}~i?™¿©K͑?ï…Zêª?~ý`©2?qp­ðô3k?]`÷œC??—á£Ú¡\î?}|ˆmH—AGN4FGL J1849.2-1647?Ø«®@çôÀdkA—zÀ9Ä/µÐ1À;áRƒZ'ô@! •ÀR–?ÿ³LØç?³Óc"ÏÛJ¿¡t=‹Yn?猪Œžß?Ø0=³Gs:?ïЍa'^¿»YÓ0C)¿åè°;Ä|¿à¿…òèn¿Ø=ÏCtžã¿ËpÀ•ÆAGNbcu3FGL J1849.3-16451RXS J184919.7-164726?égÎ?ÀuF°Ç?}$í2{"?t«ì[¡$?'˜Nb[?ÀWK~·Â?ÜÔcp#ß?˼ß¶´]?¢xí'[»?¨
Ws²¿?àn?uƒ1E?Êj}rØ¡?ëÜ~r÷™?£'éÖ-?‡ÓKfç²Û?6^¹,\®?¾%"Ÿù@Y?£0£$́è?ÝüÛð'`?ª¸>Œ;V?ÁZÉL?¢(‹%D?Ùè÷ˆú?­z¨· "ÿ?ãæ3fÅíò?Ä°Olé|?ŒéÌ·ÔD?ƒ.'PŠ?×LJÌ,?āßÿ«±?Ê™‡ÐïF?Åˁ±yí?°F¦UàI?·8æ{¡ÿ?ç}PÉNƕ?Æ|{Èð—?è…綜<?¬Ÿk>Öì?'ÈåÓ®¦?†n'-×?˯GS¯2;?«nÍL«RŸ?Ë+G̝R?¦Û‡ f?ÉÅ?öÌ6?³$DÔï{»?âð<¼Úøp?´ÉĺǡMIXED4FGL J1849.2+6705¿ïØÙ÷òY=@9
ǸÕ¦À7×Øã["‹À;"1ί%@mvK½Ä@Äù¯"?"œÃ"\©Ø?¸'t·7_@""ÇSçá@EŽŠ$¿Êƒ]Âþ¾¿à.ë¥Õçÿ¿ä»ð¶ù&¿äâ1ƒ/ÊÉ¿è	}WC´¿é%¥á¦x¥AGNFSRQ3FGL J1849.2+6705S4 1849+67?ï²õ
âÜ?êgç>ÃØ?]â¢0Eßà?`
kU¿÷;?Ñîù^-?}dž
Z?ïl²qñxÂ?®kóõÙ×?gH˜­Ýߟ?zany—0?=d0ùj?­fărÓÂ?ï>®kZ8}?•–Û9§4›?†Á՝7?²…(yÍ?‰"PF—Ó—?Œ€Ò;ä—?ïÙó·zÞ¡?a/ßçF
?Tbå…3?HG
[·ó?kÛDŒßem?Z-"lûL°?ï¿l1V.?t|–c"Z?S'îJèù?N`–3Ñër?{ek¿>¸X?r /7›µ?î°_º‹è½?°Ëwz²d?…zLb´I+?¥Œ?òfíÓ?Ÿ6ây¹'Ê?¦ËÖ¯Y?ï< l²?"ݹAS?ˆš½?—î¿?Ñ²"$Z^?Ö:¬Çú?Âa:·ÉÌ?ï€MYò\ ?€%"`¯½§?pšT9?d¯Í0̅è?‡Ÿ¨lùT?{SÛ ÛîWAGN4FGL J1849.3-6447¿ãøGÅ•ÏÀ8&A€ÓÏöÀ;+–^{¶À<¼…"êÔ@ æõ'çôp?ûyüE`\a?Ð˜'\?Ï||¨G1m@BؤU@wHÐöR?½ðÊ1u?ïãNÿl‡=¿åÊÁžpn¿»¼$^@|¿Úœ=£N¤(¿ïÿú Âî'AGNbcu1RXS J184924.8-644933?ïÙՀÇÝò?hOO"?GŠ@J‹>?<чÞ}â
?p39oˆ‡?evÿ´Ý?ï—ÏÆëü?…>|‹˜"Y?`ȇ5Æbß?c_ÿSŽ›¯?…Ùì}¾³	?'šÙà†"?ï;òªµ~Z?…eÜÏÜô?lT+Îaq?mDŒg#!?"÷%L&ˆ?ƒ¤á:àÙ!?îyŒO·¬?ƒI	å–?ƒk°ÍDÆH?iêYŽˆaÂ?£"û©É6?'ªBLÃ?ïºsòý_?rÅWç‹?XÒ{óvpÔ?Ll¢wZÑ?|'g‹rl?oó3Á‰î?îÔ.ʃ?™¨·ªâÓ[?v§ÝöÌ?~gç+†H?ŸÐGÓ½ì?–ÓDFÂY?îÓi œ\?*tω
m?q
u×Æ¥?rséé¤? §·?wN?¹DßÌçv?ì,ìЫÝ?ž/	RÆÍ?":Œ¨Kas?…PæOêHë?ºõlÔ¾?œk›Ì¨#pAGN4FGL J1849.4+2745?ѽZ*»6ð@)U'Í}åÀ9÷ö•3À<&/Ta"@^dŠ$\@¾‡Ó[?½pÛ	{~Ñ?ÀÀç¦ÂÌï@Ü \–ÙÌ@e£zîޚ¿à«Ç>B…â¿ÚC¦³]þ¿áô.`:¨H¿ç
áŒR3¿ä•îê.¿ë¬ížÔkýAGNbll3FGL J1849.5+2751MG2 J184929+2748?ïå–ßî?YZ/mÎ1?@p0Ëä"?2ë*\Þþ´?fÍ\ãZ€É?W´4!àŠ?ïύæÕY?z÷;Ytë?KyÏXÂy?V€È²¡Ög?u	ÜÕßí?wuÿÊɼö?ï"iùÖM?{|†ô ?dÜq³á?iMÚ%f?…ߺþcÜ?wxõ${Õ¤?ï…
70?c‹»ôś?eº4D"W&?C-'VVp#?‰Nî¬nÔ?bፐ'1ß?ïÉEj‡!6?iã8Gá?X"‹ìq?PE"ü6è?u8†¹(l?f¥!–¡À?ïe©1èŒ?'
pD¬D?c稜Ÿ?qã©ep?ê™…Znø?Z7÷µD?ï71D ?‡¬Ìz&ÿ?rÜÊUUY?r±»ÌŽ×P?"b¤ì²;?"Ž·;¶§?î¤ó4É?"X,)
Fc?}Êf¥ÚOV?c®aµy4y?¢cùc?ƒH¸óªpÒAGN4FGL J1849.4-4313?às
Í·ÈÀ1ÛV†''À9BT^üå™À;Û[Z™ª@Ú`	]L@úéZ¢
?­	*ÃoxU?½[3­VÚ@Kèÿ2z§@¢ç÷ ?ïÿã°> Í¿ÙAf|·¿âÃ{_œÈ£¿âAb ß9¿é'´þyî¿ÑM`pƒÛAGNbll3FGL J1849.4-4312PMN J1849-4314?ïÔ=õ·…F?q^ý28–?Q$ì`øP§?N<,í_­4?q—Êž1?nZgaY}r?ïÎ0Ê£&á?y|Ñ¿/=?R…âÆ?Y$7‡H»³?tFY—ª7î?u¢cæY
×?ïA—xhW¾?™åÏ7Ï?xÞY¯ü4?€;mDù§?'ÉYSB3?rNØÔc?ïvö£Ø.?o«_ƒÜa?zÜg÷†æ?We^='X?–4Ÿs?jÞ¯®þŒ?ïˆÚÐׯ?†£åÊ`*?hcì.
›?d©È¥¨k?‡°†'Z¬?ƒ"O4ÓZ?ïx½Þó?þ?'"újÁë?iÙHÐB??v•crIØ>?‹Z6œËä?Ž
Bh\?îìVŒB‡Ô?"J&ï–?"'׸uÁ?‡ƒ¿¬lžÔ?˜q'ª  ?h'jÅ(?포*e`?‹ÞS¦Óæ]?'H×ì,çÔ?t©ô_ø?­àÑl'Ò
?‡#˜òçÕAGN4FGL J1850.1-0758?ë<»êý9|À
½œtÜÀ9£Y7©ºyÀ;p]j>b;@'"ß @!ñÂO›I?¹f¢vb¿Ÿ 6^êNÆ?æ§VPn­]@羊êª-?퓢¿]"›¿è^ï^Èt¿ç}1¦¿ó¿ä¯'Á8¿ã€!ß&¡¿'
©¥š»AGNbcuNVSS J185002-075842?è/Œú=¸?¶9Î^'>?q>Vœ(É?`x†Œ/?ÏOa½Ø?¶'OçSHÃ?çŽh%XT*?¼K·€VI?sÈ0nü?v"*'?ДTdcà?¼óµfK0?è¥ÏiN?¬ªïÿÃl?ek•œ¬?ƒ.ÍS ˆ?Ë\ ÌB'1?«µaìÇ"›?ëlØÔÔy?"ÌH8@×?'lrv?yt?aM%³Ôêd?Á%Յ5½?"	£¥ˆ¦‡?ßø^Q€6'?À«M©´¢?ˆÆSׅœé?wX$"«?ßAoq%÷?À(ÖÏ)ž?Ýç"x0z?ÅQ1º¦ô?st.³l2"?|¿õH?àåŽ`f®F?Ä÷n+VÅß?ß`LšZ£?µ'D¢Î½?ÔK$ˆÏ?‰ÝåT×>?ÞÂs–êV?´À84#óû?ä=EìÚp?§6$ü¥?—áSíg÷á?€f,¼lôr?Õcp5OË£?¦¦"½Œ'öMIXED4FGL J1850.5+2631?îüµ}zÕ@'ÛeDþ6ÒÀ:¹ß[DÊ4À<bèn@"¾×M.\	?ú'ðßьO?ÄÃô÷cNY?«ˆã$8U?çF߂±öˆ@ªöŽ<C¿ì3q|D=?ïϤîar¿Õ—"{ªñ0¿ØGt^4¿¿Þ²qA`Èm¿Y7ÕÀwAGNbllNVSS J185023+263151?ïQº§}ªG?"Kàó=2?K9ڀ3?B®þ¥²r8?"îÜ=Ä`á?"7í?îyü¦_[?®axMÅÌ?gf¢ŽTå?qŽ®
ÙÚ??¦éËvŸ?­)Mõ_?îï2^?ŽõeN?e+Hó"h?_¹8HÛ`ð?ŸzT¨ûk¯?ŽMÚ Jã?î×HâÙ?{Šæg?¡ÝÎè[û?e×MŒÙJg?«JûX¨?'­¥¢?îïi­¡A?•å>C¼¹?Yþl¾*ƒÈ?J¼Ä%8:°? 9qŽP'?•ªžK¾$?ìžÊ3H	?¾rÆ<²?z±²g`T[?†ÃA4ˆâ?¹^"A{?½å­2AŠ~?íªAx#?ŸKs"B	?qV¾vÊl?nž0j?±™Ê
w.W?ž\ÃLí?êҍÁt)?¤Å,3SƒO?"eэs=?'Ÿ3 ºó?ÂIɓԫ?¥±·E)"AGN4FGL J1851.5+3406?Ø@ýSÛÒØ@-šÀY!À:;ţàÀ<n}'Þ[@@+0Û?+@Ÿ¼?ÈU…2à'?¹'8©ê ?ïf='u^@vwŽ
?Мöÿn5¿ëäa>y¿šW'Yb¿èÅŸ,«…¿Øò»ÈB¤¿ïõ‰ŸP'ÀAGNbcuB2 1849+34?îέFÁý³?¥ŸççZl³?GD4?:7²ÄôH?¢¸þ€ýU&?¥˜/uOO?"S<F?‰"Àô›U®?SXÁ!Dá˜?Wo/—®-?‡e'Ôf?‡øž:QÛK?ïV`j+ u?…ƒ‰%?cz˜ —€?j½úšc
?'ÄŸºlŽN?ƒÑ÷²hBk?ïŽ}ŎÑ%?dûIá?Q€Y0N?8®'×[NÜ?Š0Œ óç)?d,Èñ¶ ?ìéÃð|¡´?·¢1("%G?YaÈ(l•ˆ?OäL{æ?¸LY]G‹?·'EÃEÉë?ï+L4? ~ÑÕëÇs?e ¼<¡ó?tSîy Ñ|?*Ca[~?Ÿ9Çö?î^'õVG¤?˜»Ê#­·¼?qä.íñ?tžwüÈ1l?§ü¤!z&¡?—i*÷q?î´2{Ÿ?"­áÆuB?chk7ª:ú?UDUŽ.ö?£†WÒ·¸ã?ƒxTb AGN4FGL J1852.4+4856¿ïò)̓R>@3òÜ]cˆfÀ8ä
kùMÀ<+ÑÁÿq@±à<Á&{@ï"b*˜?£&b•K3?ª†·>Æm@à5z5PD@&NIºO¿½6‰©âg¿áŽ­½gÿï¿å§|æÛkÌ¿áõÁb¶Y¿å U—¿ìÝ5Мe&AGNfsrq3FGL J1852.4+4856S4 1851+48?ïԗtÓ<?­|P½ÅŽ?P™½èð¥2?ŠU$äÅ?qŽ
ƊÄç?§
ëUB	Œ?ïå>Á?hÔù<[?=ãS,ò¶ý?Pñ"O Ø?g)W¨å'C?d«LEe&V?ïX`í^Ec?'EˆÐg™¿?\è¤ÕÉÿ?n¢ÒÿŸ
ž?"%X
¹û/?'Ð)9ˆg?ïû 0»Î?+3ÊTCñi?!R&Å]+E?
ã^Œ›(?>}ì¼*?(M\6Ý?ïÜd^=;ä?"vøA–??; {äƒ?HµOy°07?o´="m2n?ƒåć²P?ï­á»à?‰mšÐ4è?NBëM^ýˆ?`‰· 'Ë?'£mùÜ}?ˆ$çz~õt?îëMÚBE?˜
t­cì]?e'tc)E?pÂg­´?Ÿé¸RŽ»?—­ƒ>P'?ïó œéÁ`?JÁß³ýfÌ?8¯TzÀå?*jLåX?S"çÜ®Ó?F†€»èÖAGN4FGL J1853.8+6714¿íç¥×¦«·@8£NÛʗÀ;@8
‡=À<OìTR@ z}l@($¹ó¬5?Ò¥Y€ÏÉ,?Çrç~(úË?óµZ¥hõ@‹ÒªÝ8Ö?Ò/£#Ü¿íheå7&Þ?Û5ÚØS>¿ÜóA«›ú¿ã€;ÄÒ,ˆ¿âùZ"¡UAGNbll1ES 1853+671?ï
æRãZ`?ž^Êpò?l̓ˈ+î?s‰6Vʃ?š©£*{¤r?šÐ¶n©?ïøÐòÝi?šä˵?³]ùzÓ?"û—™ðe?•b•â°?'ÏPpìãT?îÓÌy{þ?'ê(¨?Ð?nzQe°À?pþs£é¼5? Û"Yђ
?';"‡ŠC(?ì'
N¥³?'Âɾ¥l·?y¼jþs\r?b6ÕÐÞx?ºSÎÚÕ4a?''¬*ðã?í'6펢?¬Xw†çhÄ?|,®á…é?s$=ʂo?±³‡iÉÐÍ?«l:É|!?í¡kîn:Ï?°ëA4Ú|?Œ)#¿DE?•‰™b.?®ÞúP,'?¬îG¿ö?íQRNñ ? Ôc&{†?zne?~Jiæpé?³U+w‡]ó? òaa
?æAÀkâɆ?«ßœ|á?‹(è£åD_?€nQÏ¥ú?Ò£7ãBÒ?¬YËKAGN4FGL J1854.6-6007¿îÏePð;À7®Ý&·#îÀ:åùrGEÀ<¥¸	â@ù&
s±?ýâEîÑ?Ðd!s€?Ñ3©$Ññz?û¯É†Ç.þ@ÖQ·'¸­?înkón!¿ì·¹ª±?âP¤'ñ߬¿äqÎly¿àNQ!/Ð}¿ïþ\ÓAGNbll3FGL J1855.1-6008PMN J1854-6009?Iž?†ØÂ	¶sU?UeJŠ¥Np?Q#Åyœ¼?Šo•lÁÒÑ?…‡'ë`œß?ï]ˆº¼Ì?Ž««¬f®?p%™µzÎ?s§¼m<B?E™C0Ìê?ˆzšFWM?îåT-²Hp?'IIuô³?{Hì£ñÓ?~U:lR°?œƒ?ƒON?Ž1<Kaˆ?í¨/ä@©5?Œ¿È\™–¼?€Û³Ê9K?kõœàÝE?°£
f`\6?‹­sw8?î­ë§S?¡€çºòS?lðºPÄå?`ä‹K Vë?£`埶Ñÿ?¡O	è?î/–Åm¡³?¨"½ÞU1÷?'!€ÀÉ ?‰p‡ö…¸#?¨fKLOQ?¥ |KzÞ¶?î™$B™F?›"­¾?@MqÓ¤ÿ?€$¤ìàE×?ªÆZZÔß?˜Ë˜›øž?êBô`º€?¦û†KB¥j?ŠÀ݌Tåõ?î9~ÝÈÌ?ÅKÚUîÁa?¦yRƒÆÏAGN4FGL J1855.8-2028¿è‰%µUÀ$<âó¾ýÀ:ÍËÕVJÀ<>¥}Ójv@8£ÆCEÐ?ü{"¤£?Ô%ߙX+?ÝÎÆâ}
G@¦ò¥¤i×@	%rÒ/6¿éŠ"XŸÔ?ä¸Q€%TM?î¾h›Œ¹¿ÐDHÄ¿ã¿éåBnºs¿ïüHOúêAGNbcuPMN J1855-2027?ï¸í`§?˜€ûPJƒ?g_¿rÐ?h 9¸´Å ?™GveÀ?–S¤4*¾•?îS·º8lû?´
k´¡5?g¡º:Ô^?xBiÇËí?©JhºÊs?³B¨ÂO?í=-'Üû?¡«One(ó?';²€Ս?ŠM%Áé?±Ç«3»Ç?Ÿ&"κžÞ?îp ¸¶"%?(½˜°Ð?péìrx{8?`³í#úœ?¦Ø¶åÚºÌ?Œ'÷nJ±5?îa
'¼A?¡XLÙ]»?}u;`Iž?{ÐN|½2?¦9Gï3Ó7?Ÿdç‡Ïqâ?쁣©%Ü?Ã\ò÷PPr?v;ëh™G?‹¬¡Ùæ+?º'D9چ
?Âÿ'«S'?ë¿kvÎ?«xâÞ¿»?™Â†µ¬ÃÅ?'9µ£þ[í?À¸±{§Z?¨ãÑGÇ#?í'gÿŸï?¢¦­á°­?w3ë¿'/?s‡öÙ6¤Ä?µQ‰,áuÖ?¢ºÅí˜EóAGN4FGL J1857.9+0313c?ÙD*Ñ(ÀØ?$yςgÀ8€Ä0FéÀ9É瀭9Š@󾑠¦Ô@oÃzn?Ô¨(÷?ф(£ãž@	oŽÀøƒ4@ˆLôzeÍ?ïM›^•·¿ìMè@EÀT¿áÁcâþ¿çª.£ˆ0¿è°KŒÆL€¿á_#a.AAGNbcuLQAC 284+003<?—ê
ˆš?š©èù­Õ?ƒ]J¶?ˆ5•Œ¿?îòyӑÉ'? ˆË/º?·T¶¦õÁ›?¹¹ɪ6(?¤jE+
ù?¢"%O+?ëÎÀVêý?»æÂc´§´?¾[ؘÝÜê?¥xãuîŠ0?½¶¢Ë¾Ò0?¨¡Ù܏>u?è}°"õÚ|?®Xˆª¤|ù?©ÀÞEßÍ?'Ê4Wz¯+?"¶)Qšî?z±s5oä?íÏ~@ÞӜ?•ä¦"1·?ŽÏU¦L?ûTÛµ¯
?‰m×åR×H?£­JáÍ?ïI›e³?¥¥d™€Ç?¦¯¨ÑOPf?¦~´Ÿ"Õ?§Œɑt€?©Æiˆê%Ì?íEfD5B?±Ë¢UÂä?¹Z.ç_zX?¢ëw#ê[?½Å"çê6?§­¾/IE?éÅí"?­ÇyB?‹XÆîûñŠ?yŽ ÑG?'"Ö[øÁv?'­@¶m«¥?îýþ1…~?‰Ñ£î~›OTHER4FGL J1858.1-1821¿º¢LŠaDÀ#]FÞ	5À;¯¥t™/À<)ñTk'@ v‡¬‡2@
 >ÏH¨?ÌǺ.d—?–î$"æ°?Ð"g~>tZ?þ6ÍVWP?Õ_"¥Fv?ïÈ!‡¿¿èxpT%ò¿Ýùu3ܦ¿Ý¤çá%If¿åŽx¾­¥?AGNbcuNVSS J185806-182314?ëêr4OèÌ?³ðö&"<®?eÍY0¾#ë?[H_·—þ±?¿þ•O¡Ã?³²t{ºÑò?éó#´BÅÖ?½Ù"+À›?pqN}
ʎ?y0W=V?ǯæº++õ?½]9le$?íµhQD›?›¤ÀÌàÚ%?tc®IºÃ?gñº½·I?±2¶y?›;/K¾?í™*ˆêŸÇ?‰ólè™X—?|î';‰h?bÎӏij?±vœÔâo÷?‰Z-
3¼n?ç»?~ ?ÁrÃæ³m?rC^\Ô?elêr"Õ?ч|—±Á?ÁM/±|?ä]L²òAb?Èö7ν+´?v£¤æ!>?ƒÑÊðwŒ?ÖêØwút?È´h$ñ@?éÅ>»§‹u?°ëá:(?…"ÓÛ?s@Á÷ë¹?Ǚ³oف¼?¯8Eœ»cÎ?鲈ü›úû?¢âƒ)ñ?OÙû?}+eì¾d?Ç4+P»¯?¢«ÀÎï'AGN4FGL J1858.1+7318¿çØòr×@¢@9k©Ÿ¡—À:qt4…BÊÀ<{Tç4@ôœDCѼ@…w£¥Œ?²{"O…y¿¶lþ[EB@E–È.›@_ûé
¿áˆØÖ+¿ãMMüUy¿íMÖýÓ*	¿ÁÔüÇuC¿Ú{"BšY¿èê–o AGNbcu3FGL J1857.9+7319GALEXASC J185820.26+731714.3?ïƒð«Vãð?‹ÍÂG"?c
ó2e ¢?Z8«¸k?Š@XZ–Ú?‰œ·"ý
â?¾NÀé?•1‹ +¯á?nù}Æ.–ú?ˆR‡µŒ+?ƒœpî½}ó?…ûôÕôù?î=ti}?™Ž,¢!2?€¥*¾k?'gÄ[£b›?§ÿy÷›?—Bœþ@Ö?ïsLaò'>?r'Hl€[Û?r Ž†¼*g?]ã"8Ò6?Š FGg<?nI"ç>E¿?ïYƒ»?›>ǛGŠ&?y×ùêOß"?uÅ",Og:?–†¶NAg»?˜=+À´KÞ?î¼7«gø?¯¡´æ¿ Ä?ˆ0¹±~?¨ŽIçýD?œe¼…Gv8?šD
 ýf?íNMi{€? '«˜)?ŽwÓ(å?Š´
îé?±·fš¼úà?žÅa¨Ï]?íå'æXb?"ÒÛ0r Ÿ?•cÞo®?‰§¤1=³Á?¦õW,""?¢Zž·/AGN4FGL J1858.3-2511¿À/ÿ
À)6~À¨À9!áKßÒcÀ;§5Þ^s@ÈWC"?@µ»8OÓ?±¸põ5¡¢?ÉX"*ø&@e8}@6sšœ³?ïü··ïÆ¿ßÞT~ÝU±¿åN¾Ôçx¿ä!H2ž¹¿êª¡Ô¦‹¿ïÿCAž0AGNbcu3FGL J1858.4-2509PMN J1858-2511?î%Vô8?ºÿ¬—<?¨€qqµ¹†?».q†ÄĄ?"¨µ®\¦?{à'qÈv?ï›nè¸]!?Œ}Æ.Â?e"kOò²?miÎZØqþ?ƒ¿*øÿ7?ˆõ–màÆ8?î<]Èvë‰?ŸÌoæµÂ?™ 1DŠb?• bÓ¸8?ŸT5Èu
?"³|dl ™?î/Ô©É?Ü?E5?‹}wD"Á?i—üô¥^?¦#W›bë‰?{¶awO~?ìñE¸¤Y?¶þê†A?¬å…ÿ~'ç?²Ê‡¾0ïå?¤v9wƒ?¡Ó¶"E?îòç'Sˆ?°­1ÉH*?†c[(¡ˆ?«e‡ôI¡0?–|•ûÐî?åÞS£dJ?ì> ú‹ø?¬8«±ð?°cYF¼S¸?¤?NϏØw?®õc_ný? MÓ9Ñǃ?ë'¯«ºë?—e4M"§O?¤~¶¬^t?…À"nÝ9?½Ä«*»•m?"µ}wel_AGN4FGL J1858.3+4321¿×"zŸ>°@1>ž¡À:±Ðz×6³À<‡©qÛ@…z±!@›¹!]¹?ºH¦7Û?±¦ÿ!¢€ã?ïÁŠ¿66H@Ö%f
?í}Zi"?АC¯'9+¿èqÿ¡¶I¿ÛÔS±Wü¿ã€§û\,Q¿ïÿÿÊPËAGNbllNVSS J185813+432452?﷋'N¿?pÂüé›÷¯?Y$£€?HDÍGàôx?}ñMƒÃ"è?n:2
;J?ïO(ˆEšz?"Ãú™£O‡?lߌ™Eò?n$>¤³Ô?'~ý[ìØ?'‰•lB±F?ï_À±O]?{aŒ^ˆü‡?lK«hÅ…?d@—GÎV?"r{8(½?wˆ;žtÉM?î¼,©ßÀx?w*ë7²N?ŒäW™Þ¨?j–†£€?š`bk¤?rQ'<pË?ïwKŠªh?'EhšEE?io;È;AA?]¢Â'U:l?‹Ñi0/¦?€Nʚ@Ô?îG|«Ì?§k÷®ÆÔ?†6Dö?‡Iê­þîm?§Gžp¶#þ?¥•c7´?îÍcƬÙ?ŒŸôSXÕu?xžº²BXÒ?rdÅZI´? ì=ßZ?ˆóÛ3¶É}?쉂sþ?'8aO¹?£Þ ò™ß?†83:NŒS?±Ä›ëå^?Œ[MÞu»AGN4FGL J1858.5+0640¿Ù…ìFBb.?÷øZðŸÀ9›=EÀ:…õ|ï>è@ ºu\M‰@F49Ãp-?Àå13ûÛ¿EłVž@[?çK©!?Çæ{Ÿˆœ?înÊî¦;i¿ì.KlåÜ¿å
ÃþGB¿áqüfîK£¿á®M?ùÀ AGNbcuNVSS J185831+064016?æ¯à5"?¾™iâ·?¥úˆ"0œ?ªü
)´
\?éÝmÊÄðò?«ԧ1?Ҟ.¸¾ç¡?ÌcÆÃö¡?˜ŒiÏ4W·?œ"…Ü"·?åì…TÆ´b?Ì"ê5†?Ê·y79?¯,Áч?²>qÁîŠR?Ÿîw£lڈ?ç
S'«bç?±ï¥w"ø?Ø¡Ó¶Gÿ?°'ÚÉËÍ?"cTNûž?sXå«´?ãû'l×D?°ÿÏh…?¸f{ûr(?µO«ï?¦–¼A$¾?¥.R¢g?ë›Iļo?ºT"^i?Ï,AÅzы?Ä}oÈËòn?˜ýL—>gÈ?£Ys]RÔ?çm)¾?ąkÞº#í?Áq÷vþ?§Â¶RÊì?³ô‡1$I½?¡¾Í{`'þ?é$ñ< uI?®ìØ/&j??ÇÒZfg?«rÒf[?5·É¾j?†Ci츙?é!»¨|#?¬ô­¾ú8OTHER4FGL J1858.7+5708?è‰yL¶Ö°@5Ìÿ!³¯À:Æ÷–¤ò"À<¥¼ä!}(@ƒ¹ügÅ@ÉYø™Ú?DZ~è"Q×?ΫúÅ-œ@à f§ÔÆ@oüt°++?ïòæ§ieõ¿ÞF~1ß ¿âxP©e¿w¿Þµã¼¨gh¿ïñIï7Zà¿ìY? (ªAGNfsrq87GB 185759.9+570427?ï`;ø\PA?'‡YEٍ?{áØÃí'{?mÌm"Hšû?Š|þ~,?{`Ñg\?ï<s¹¾°³?"Ÿ˜úìC?k[kR2Ï?‹>Kh~܎?w¶2$d?"0÷X¹m?ïPH܁?ŒÅ‹{pO?…Íf™)^?ƒ€N.Ê?"ïCš3f?ƒU?V'î?î¦Í¤ŽU?{N"A¦Í?•5Ïí)è?r̀Apó?•ð{‡óše?qÂ~ˆ"Ñ?îx™Þ|¼X?—iû¨I¹?'-BÎôª?"<ÐÚêB?žÝ–òÀêP?'¶ÖÞØ
?íôB!™[?¨œÄgë¥?•…æg?œhËpGh?¦7Ñ¡ŸÎ?ŸeU*±?í²%±ëJ?ž­îé–×Ô?šÜ‰Ô
Ëä?'‰Ô¯¹#t?§o_ø!à?•5ùǵ>?ìkr'‡?•ñ`Þ7?ª-vÌ"?Žµ«s
ä‹?¯ÐaŸÒ?›ŸÍ˜ØAGN4FGL J1859.0+2329¿À™-ý®@!ÉdobÀ:M¼àÆ~ÕÀ;á<aNÏ@F×zzÅn@ã `ȗ´?Á,C܄¿€fX¤†Ý?À§H®ÅzÉ@Õ;@ráÊ?ïÿŸR@>´¿ßqªgG7¿èí5" ¼8¿à¨>b'D¶¿á¡HÌ!¬¿Ý¤ëGWAGNbcuNVSS J185857+233007?éW։Ë+ž?Á á}o'¼?{:VkÞ&½?nQ,Ta¡?ÉÆÓ%Mä²?ÁW";‹Ç?çÏ/?U!è?À±ëî`'?‡ ÎÞs3?‡mbÑRåÍ?ÏQ628¯?À–§ïB?êñ"(°<7?¦1™¬Ä,?.ƹx·@?"	áÍ?Â3ֆ´åz?¤¹CƒèvY?í×jžjŸí?i
ƒ8…?zY\*œ?V–zEåi0?¯>4
wþ?€‡Ìzßõ•?ä¸X²¯ÑP?ÂÔFø¦´#?Œ4økL}?µG^5x?Õ­¦Ú}m?ÂÎqŒ#(=?àÝqµ¤è?Ç'E©?‡ _™^.‹?Û€mtP?ß3B'Êü?Æõümp¾?äÓb%,i?².3J(né?¡©à·Ûç?s[ѾÍP?Ô5¦z¨'±?±ê
Øó?鳐WÈá'?š&rà'2"?">W?D ?y¾Íèüf?Æ©ó¹  ?™IóEâ€AGN4FGL J1901.7-5140?냗»·ÀeÀ6{þ;â
À;FÔánDÀ<µgÓMðN@nl <K
@è"úô'…?ÓÁi¢#?ãgþFÂ\@
0¡C§?ó ·?ïE´À¦Á¿×Ñ¡³CŽË¿Ñ¬ÿuìk¿äbÆÜ	¿íÇ4—ɶ¿ïó_2•AGNbcuPMN J1901-5138?è5QE—å?¾ÉÇÊ.ŒÛ?Ã2'œž~'?¹Zi¸=d?¹z;Lj
?°'´ï+3š?滏9½?ÌÕÀÉ*Î,?ɤQß×Ò¡?Ⱥ›‹¥ÿÈ?¶Úão^Y=?±ê$Ôÿ)?ç._&^Â?±µÞ@4?ÀVn¨P?¦röÝ5ˆu?ÂñOÝ|·%?ªnƒ)5pŠ?Ük¹ü)u‰?©9œÏq&?Ö°ÙƒI?¨ÚBÈzÎ??ÉÆÙߖ[?¤üÉ¢rr?å¨"}¥¿?¿¡FĦ?Èô–äÍ8q?¼i¹hR5?Àjß$›ÉR?±x›­?ßkۆà¹?Ò¶9U"º•?×AÅr:…?сMùÄ7ä?ÂõÅg[aƒ?¿ÁÅ÷_a?ãœqç½­º?·»ËIâC¤?Èi¤v
ð¦?²í¢ÄáR?É$"í!ð?°‰G3?É~ÍñÝJ?¥J^è°G?ÝGeTºå?·¤çƒñâ?Õùê2Ÿu¸?µ €~'¡aMIXED4FGL J1902.4-0629¿ïȨÀŒ°À‡â`²È?À:Î-À,«ZÀ<sY"ð@!¬Ê†?ÿ4«ˆ¯fŠ?ÇSŠI{õ?@àWt7?˜4éÊßb@%'}?ÚµŠ;Þ§¿æ w~瑟¿ëB1}Ñg?§­?·T¿âøô=Te¿Ñ¸#@¡ÜAGNbcuNVSS J190223-062850?êBðuHy?ºí©óü3?iR¨–§Ý?aÅ;0G8€?Ǝó‰‹?Ë?ºÆÜ)Ùd­?䣞$DÙ?ÄÑì~	?x3"IJ×?'€ªšÕÒ-?ÖXO''r?Ä~¢FôË?ì5ì»?¡êgóq`Ç?x[•¼8)»?mŸÏL.±?¾X™¸èL?¡É ô1Ä?ì®À"Öå?•ÄôÇJ?qÖh~"ð^?['PcÀzÌ?¹l˜`‡ÊÒ?•£"
P…?å‰ñêú›?Ãê¸äm?u»âÿ%;?kˆü'>?Ԗäfä?ÃÔìiþª?ٔ™ô¢±?Ƴ×rî	3?wH­-ù*?†7v¸
æ?ã!«\ Ñ?Ɠ¦îõIK?çbÞá;2 ?­a3µY֛?…‰ð´QŽ?z¸iY?Ѝò¸UË?¬Ù@*j÷@?æ$
œn¾­?°ªIŸÜ(à?‹Ûê™&´?~fWà ~¸?ÒÙqD³0?°"u`
ã—MIXED4FGL J1902.9-6748?àX¼SF½ÃÀ:$咖pÀ8ðÜùjº‰À;ù$(Ô4 @¥Tƒ™@¿æ4|ß?¦O§!wþ?ÀǃwCXo@*Y:-ù8@‡)ÜÈBy?¯åµüÑ¢J¿à›NÛ/f¿ç')oe©¿è.¨>Íñ¿æHp¡þ—ö¿ïÿÿ^ðP`AGNfsrq3FGL J1902.9-6745PMN J1903-6749?ïîëb D?Ry(ã1"Ð?FWŒSÓ}Ü?<€8h—?XÈbÇ*år?L¯M"•¹D?ïê.ѓtÖ?e'°"!Ï<?4cÿ6?AA<dCF€?cD®WW/?bçæLr~?ï—Ïj"|?ƒó/":·»?kcŒ
¦A?w¯º'ÂuÀ?ƒ3Bd	?€
m™Aú0?ï_G[?@}Áp?tû?=#¡ñ±?%¨ã:õ%?[K+ôæÌq?;-ØVPË?ïÒíµûz	?kËo¸ö/_?S¹ì7…¯*?K4ÇQåøŸ?qš©ããoŸ?h.4v¢DH?ï½ÝØ&·?l3T=?Q¸½Vþ6?bÊwÙ½u?}3bÄJ',?€VqvóÐê?ïv%F=?ˆ"rÈ{X?jrK'{ð?uê"`Žž[?‹ácÛè5Ã?…DC}‡X?ïÓæ>ié?`ûïÞÍeÜ?R΂Z;ùi?B(=µS^
?qY@Dßõ?]?‹^­gAGN4FGL J1903.2+5540¿ÚrKþAu'@4ˆäC‹À7òË/=ÛÀ;oáÔï@gÙØù×?ý+¡nz1?™(Aà ü?µpþÅÃC6@RP.ì|•@öfÏÿ?ïý& Ñì¿×«$˜Æ5¿Ü#Q©ß¿ÜK3o™¿âê+íĔ¿ã…]7»ÄAGNbll3FGL J1903.2+5541TXS 1902+556?ï¬r÷O?¤fì÷yCš?U1Å9 ƒ;?kM Þc£k?'=?àB…ï?£ôÕY­(?î'üÕå5‹?¨^Ï%9ï?'ÎŽ¨UÈT?¡/¬Ôª~Ô?œÑ֛†Z?œ/BµG¥$?îÿ»6;??—çȚ›É¶?Ê@¶?"ôÜa?'#›‡ý²?q:áŅÅ?í:Vi?'%f4õý‰?™6¦›Üå?}š£¯È;?¯¿JÓïÈÿ?²î[;/Ä?dŒF ?šËËèBÁh?[óërû?fț,qC(?ˆÕ…`°!¤?˜˜&-åa0?ìί"Çg?Á#à{Ö:?©¾/AÅý?¸Jåq'mT?²Zs8áÌ?´ÚDž?ú©ÿÃ?ÕÉÒn
?êU&€¥à?'ésǃÌ?™cë‹™®?"W²¥vu?êQó!l®¡?¤à—ý.¶Ä?§½Ø¤Wžß?'1°÷æY?ÀȽQ7]Ã?£ÒmåO"WAGN4FGL J1904.1+3627¿ÏÍÊZ¤Ô@*¾°1‹"GÀ9ê7iDÀ<4†6††@ ÔW§†Â'?üdÓSϊí?µÒ
_š~?±õoÙ+ÕÇ?û£¥Üû(@³†;B÷!?î[?î¿ìêg‡?âú°4撿Ûsµ"[ÄÍ¿Ûk:v"¿âQ¼‹6)ˆAGNbll3FGL J1904.5+3627MG2 J190411+3627?ïÜØ-Sb?m
$"tv+?,"t ô¤P?ø"ÒS‡?p²ÕÉ®[ß?l¹W¬'§^?ï¶ç—B@0?‡"E[y¯a?K®ã8%§?UaŽ6£Mø?€‹+óÈìó?†M춻Ø"?ïWÙ¶?"郊æ,Ø?UÉĮ̀¸ç?ac6ÿæ?ž˜'¾î²?"›üØ×|?ïJ[~‰{r?qåYŠ"®ž?[_ô×?DW3¤²ž'?•O¨¥IR?qMÁ(§³?ï»:Y©OÖ?y¹ÛÚbá?>QìW=?0›n	½V?€>Ú?(ðF?y%Ü*WË?ï9­¿Q B?ŸÓîK™þ¼?_iÔøÇÔÏ?onÜè´ðô?–ÓªÌÐn?ž…泐?íâŽN¦šù?£Ï¸èÓäO?[/éWíÓ?WØ߆4 g?°~ÍæRYê?£Íÿ*V»…?î*ÞêðÄ?I¦éÐ?o¼Ž•÷O
?bV›2Äúü?«VHuµoÖ?ŽoÚ	t""AGN4FGL J1906.7+5419¿ïõë[¥(@3œ¯¢ðZqÀ;"§z¡‡À<Ò.d—YM@×3ÞLQ?þy™aܔ?Ðý'üft?à'`ç÷K@M;å‰\5@ºÂá¼s
¿äžðP_"ä¿áûR'L¿Ö#º"ˬ;¿áÁI̽¿ïÿÿ)@k*?Ì=Å]l¡AGNbcuTXS 1905+542?ë«ÄÐÆ¡?Äðó±4Z?©–ò4
Tµ?³Û"ÐÊ
å?µÖ`d蹝?¾öp€p?í|áüΌ?³&ِƈ?£Á4?«
|ã•?¥/rͲ?¢€Ï߀øq?éåkmr…j?©1"7k?¹Æ¨'Ó#J?¤ì«lÆ?·
üPe? €‹I­o¦?îuåhÐ?…Sfhñ"]?•`˽pGí?uãe
Í}_?¤ˆ;Ë£¦?!5w´ª?çq0P)ä?ÈÇêHuÿ?º%¬Àp{œ?»gžÓÜÙ?Å)à¬Ü?ÂÛµñÓ?êDvgƒ¬?ÀSƒu?ó
?¶{›/?ºÎđÈr~?·ÅËK6lö?¯¢æ¦?æ»ñô,?Ø?±"
ìö–}?ÃäógÊ?­nުу?Áø+J[˜Ø?¨Ãòõµ·"?ê‡Ó¢:8F?¢Só£Q?¨1l¶A?'N=‰}Œ?¿¨¬"é£À?œ¤µµŠdAGN4FGL J1907.2+0126¿º+T­–|ÀãªÿójÆÀ9Ûe˜áöÀ;r^‡tÔ@ lû™¾Øm@WhY…­T?Àè%ü¾Ø?ìá~à†?цW2üÂ@ uT•Ùq?ïÆÏ\Êr¿ê0¿»lR¿ÛåÞs=d¿äC¸§Ò¿ê¡É´˜c?¨y?ÜäÇëAGNbcu2MASS J19071198+0127091?âÙʔÁÌ?ßú¶õ˜?zQáN†Ï?p¤–o:õ?Ùã#RŒâ?ÖIM9?å>²{Ey:?ëtO)«B?s¸®èú?£?yOûǵV|?Õ3¸Ne"®?Ã}'?èòf.)«l?®Lå5ú8?'D¹'z?‹«Æn$P?ÉíÐ#Tª
?¬¼T¸Ã^?ê¾ÄŽÐB?™«Óe¿¸Â?{\¬Nã?]Á˜õ-‹Î?Ä*bá1ð?™"¿Ðי?×zµu9µP?ÂS¼,cÏ?Ž´ú
W"Ð?…%4Ù+?ãÇÑ]UE­?¦Õjøi?Ú€ƒý?ş ¾æä?sé¯Sc®?'¼ÿ†(ó?â̞a)?ŕ"­²¼g?áH){2?·+"ÇHe? zŸ¥Ä——?'ÎV…_àA?Û`YQT©?¶bCöÊ®,?ãK}‹a?«;~ ãȎ?î»Î¼ç?{Îüxq5ä?Øi‡Xà?ªûÔ#è™ZMIXED4FGL J1907.7-1232¿©dtêOÎüÀ"'ãâ"À:|Á>úÓÀ;Ç0ÄÃéÏ@róÜ[50@e*ýÌ=?ÌBÀÄÖ´?°Ïѹñ}Ü?坸ýâïN@4"û§Öž¿ïþ{€©Þ‹?ïø¼©¹L¿èŽÚù¶9ã¿ãlžä²¿å¼ôýîWâ¿äo åRÖAGNbcuNVSS J190748-123221?é'iªú¦5?Á¿,÷Àýr?s>ž	¹'Ú?m¬›$™G{?É\dd®€\?Á•ÓÖB:?쇍Ðòv?µ¥æ½`?d+ì7ܝ?p¶bkœ¿?»">«Öª?µZïòŽß?êI£Z–,/?¨OÚ@¥M?"ŒÒº6B?‰eóh±´?ÄGØ=»™Á?§Ÿà&8&w?í¤l²õz?ˆÄ£ûEª?}0eÿ0rÊ?^‡4F>ŒÝ?±	"YFµ?‡Pô{Á&?æ·€¨´?Ñ8Ädõ?ƒÀÐ':Ѝ?}.2å§Üu?ÓRŠ~&$?Þ"Èà?ç…Úv1Ø?Çö+±ÅƄ?}pÿ"ž.?"?¦v0dË?Ð~‡ä4Ø?ÇÉêoJÄ?ävL—!3?²D]	íÕá?£¨˜»ÓIK?"À'y‡úb?ԞS¹KÌÃ?±R{Ÿsþ?ê`‹8ê$?¢'§ŸÝ$?ŽûCRœ!b?všÝð@Y^?Ď‹<oÙ?¡;Xó@'ÜAGN4FGL J1909.5+3511¿ê:MEzð@'µI@»±òÀ;s•ûg¿À<«a«Ã@"•M.²?üzi¾	»k?Ðmµe'!,?²uÄ'aÿ?åP¾ÉÔÊÈ@óß+ôûj¿êwÄ?ì"Ô}›6¿½Mߢú¿°£ýöjœ¿èžHUh?ÐV±Ý³$AGNbcuTXS 1907+350?ïÌ5+l%©?wۘ(í•]?7HÙ¼þsµ?/{+õ^¥?xpÜ°Ë\†?w[¨—kEŽ?ïXb_EµÂ?œT3~Ÿ§­?U²E,ž?a'6
ïk_?"˜Ë'ú"?›YSŅù?ïlY"9?l{tw?cļ¦@?dÍ"ã"ÝL?'¸âz­?ŒSîÊùø?ï_ˆö«Þ?sëÈ¿àÍ?\z¸OM?D°Â€K?'G5¥|œv?s™'Ònç?ï˜-¹ª8×?"¬çŽ ëh?G–2ꊎ>?BGí@"û–?ˆ{.fÉ!l?"-J[
¾?îˆz""˜?°ãWÕÌG8?cr~®ûæI?tï"|1?¦A6Ä÷¼?°xȂK…?îײƒöD?še¡þ­?m! ÚB»˜?nßðÖðNÌ?¬ jÈd¢?˜Ý~	–ä?î.¢‡ÔË?'_p´æ)ª?o)T½:–P?bàøQڙ?«#B7M˜;?'FS'ñ†JAGN4FGL J1909.7-2140¿ìû%£†5À+BªŸ{À:1"qê('À<O σ`@O'`Âãj@@×¾˜V£?ÄÏr™z?º=‹ÀÔ›?ôîÊ2¾™-@Àö†""ù¿ïÿæ4|ßO?ïÿ=ba(¿ä¼N/7ûð¿äŒ–ç7²¿ÜM Å¿ïÿwåëoAGNbcuTXS 1906-217?ïa«"c–ö?†#‡Aô?d˞¢¨A?b(ºˆûZ`?'1ŧS;?"x˛"ãM?ïËõ
!•k?~Y;Ó9QF?ING3Üû¸?Pgâu*Ò?vÛ°˜Qr?{ԗLZr"?îW.;–s?–whŽ¬"*?"Œ­²;?~¸Ø'åÎ?¦FÙò
ôÁ?"™8+ݬÙ?èl?|&:¸Ëֈ?ué"'¥u?Z~05¨Ñ?¡a'Œ‰?y_pÍ£Y‡?îVV9ƒÀ{? UaXž?†ñ'Kº·£?†Öa
E"³?¤Þ;ÔÕJn?œ‹áß©Tj?ïg$hü)?æ‡³Š?b¦ðÀ­Ø?o
BŒ"¶?ºý]—ÿ?Oqbñ?뿈¹?¨ž¢´H½ ?•7÷ƒ¨Ã8?Œ>}2='q?¼¹UÙrÄæ?¦LјM9%?ìô‡«§Ûs?"»>]rr?ˆù«.Ûò?t"‹q	÷?µ<=Úoç?'éJnԘAGN4FGL J1910.0-2453?îžèÜU‰}À-Ø$xGÀ:Š'Úb·…À<+¼•G$'@Zx¥-K"@sf³"@?Í¡¢§ŠH?ÐÂ÷+c±@€Xeã‹@©‡‰Ìœü?íÏ~x¿äò]®î?«ªÞU؜¿éRKý."h¿î±†Àyt¿á"Év7AGNbcuPMN J1910-2448?îâ`7Ö¹"?–.Y½Ù?q'¢Ød¹?d©gi‡e?ŸOP`š¾k?•Mºÿâý$?ïk©bÔ$t?‰¼^ÖÕ-Q?pßD¥?roìKÁ:?Œ¦&¶FOO?"{'͐D?îâìÚð?˜ú"-ç?"?1†DY?ö>ä€î^?¤Ÿ9XVm?'pêC˜?®?íµ!À¢¥?‡xÆÔÿåî?ŠQ¾8s?o£³ÊW‡'?®(O†NXì?"3SÊÆwõ?í¿ÄlÅT?¤Zl?ì?'E^äý#?w¦žzK?¯raºbÅ{?¢ÐÜ(™Ù?îiÃ3'º?¦\sjÓ*?ˆ™]{߉?'°bNwÞé?£aæp?¡ŠãÖÓ#?ì –f"8?£x¹o	é‡?£ 
úZÙ?–§$U?µo¼MêÙ?ž›Ç") ?êy4פ8? £LÔL¦?™šÀÃёÞ?Š‰—íÓÌ?ÂçԋÄ*"?ž'd~ÌÄAGN4FGL J1911.2-2006¿Ø­PôAäZÀ*v±=û
RÀ7΋8§À;<18‡0@}ædÌ@×Å>c?ž_ßÛê™^?ŦZݜ'é@$±Ë«d9@´œïd|V¿Ì8Lw§×J¿áÎÕ»ˆ×ª¿æ<tZDïô¿ç{tëdg‰¿êÿ`Ónu¿ïþê šª;AGNfsrq3FGL J1911.2-2006PKS B1908-201?î<uÆÍüš?«ðñÞë ? ,»¼,Œ=?£Y?¸+ôÞ?˜Ϭ/†F?—Ë	"'?ï=´Û-R?¯p8Úä}ô?Yî³?™î, Dn?"ÖEÝ´ðp?ªüRCÁ6F?íI7!\úŠ?¨ã"yjÝÁ?¯ˆ¼Uõð?¥Wqÿ‰©?—É
XE&Ö?–®¥œ8.?î|3ÂáM?'§´ؾ?‹½¼MI?}ÃæU©9©? ÿIÐó;æ?ŠgO« –?ìö	;h?² 'ì"ØT?±}8ùÿ\'?®kEÊïºÔ?›GúòMZ"?—ea¶Ù?íî1*¼¹|?¶dáÓóqL?ŸZæ/Ãi?²%4übÆÝ?¡o­\Ñ—?¨³jŽßÄ[?ì)+1~t?­SÀVÓ¾‡?µP\óº¼?¨ÿéŠð?¢Ì'þ‰?‰²⁗?ësú[®Úý?¨ÄFŽ¾?¥NDR1©…?"gõg¼†?¹¹
ù_×?¤/wï7~AGN4FGL J1911.4-1908?à(P0NZÀ)Ä£çÑ5À9²×'2tÇÀ<"†4b@ ÁÀÓg?ýªbªCž?¶ã´3gÈ?¢îbÁýL?î,ný@	-ÆJ|¦¿îÝ2K¬§?ïÕdž½Ê¿Þ¶BFÌm+¿ÚNï;â"D¿Ù˜j¥:a¦¿ß'%¡ûAGNbll3FGL J1911.4-1908PMN J1911-1908?ïô×íÖ÷?LYú,Á-×?#ì=YÉb?ŒÇùÍòë?T`ÈL~µ?JÀD˃n?ïé"u1I=?qÃùé_Z|?1"©öș˜??´¹íܑ?d:õÁX?p_6>ÓìÑ?ï¢ےQ?vçê®ãÄg?TE@Tņ]?Bem·Mg?"öQ1t6÷?vR"¼cé?ïuH&4r#?f5¢Ö²?`{Ü-°3?AIü)Hu?ŽŽÿq@³D?e"{²[è?ï쨶SIå?VÛ?šrL?6˜ÂQâ¤×?*<8k/'?`"1þ?X?TÛLC†Ü¸?ï¼ ^¼›I?'îsV2?F‰x-4nF?U«î¯nâ?¡s Ê? i>Íc'?ï]L.#?…A‡[iã=?_ÂX°6'?bE]°žéœ?'`Ü)ZC"?"Àáw¢Ð"?îÉ">ú£?€ú²BšÊÀ?qû2Œj?[ƒËh'Š?¡0!xÿ"é?€:ke›'ŸAGN4FGL J1911.5+0311?íÔ[Gµ‡rÀ-<ÿdύÀ:¨ÕâDiÀ<"y™I@!–YÉË?þ,\\×q?эM{2ü,?ÜÄÑ¢@
Ö0'?ûóHàn•¿çzá³
Þæ¿ïÿØÝý Ó?ïýÖ$dcW¿Òç*{Ԍµ¿Ùi>›A:¿ïŽÎd|[AGNbcu3FGL J1911.7+03072MASS J19113134+0311093?Û5'3Á?ÌÕ0pòB?ðê¸Y?‰4ÿÉËÒ?áí°?"²?Í]1
±VF?Ü9ñÊx®?É%OéÖ?' "Ĭëü?"ÞˌaËî?áRV	?Ƚ%ºÏŸ:?ç?ñÔ\ýÌ?±ÏŜì?§£Òñ`?—"Õ³§í?ÍTx…ÖL?°æ2þžÅÂ?â³×¼J°?­z1Ü\fý? ó쥞úE?Ð²Öµ_?ØyÔ9Jù?®Mħ5ú¾?ÏTŸ¬$®?Ç•ÿŒŠ?"°q>µ,?"KÈ^ÍR?çT‹aa^?È·Dû1º?Éòvˆ%0š?Âϙ¨­š? ²¼úHP?§›	—i¥?èx6ä7U?—eL_ÿð?á¥s¼‡§¡?µyÏ2"kó?¯Û†Áo‰?¡©F•"­?ع§ÅÆ-?µ*Ÿç(¨?ӊ½Cþî™?³ÿWxyô?¨VÄÙtŒ*?¢æå8ê²Z?äµ5$‡Á?µúçБÛéMIXED4FGL J1912.0+1612?ê–¥F9å@¿2/'À9ê#'¬?À;3³ÍêÚ@Ùà†"@u±ã<zÛ?Òl¸þæ?ÄÕÄÞõ?ñ'þKÊÙ®@<~€¹xÝ?ÒåÇ5樂ë¿ãåî¿â{G¿1X¾¿ärà цƿè‹6"çƒ1¿è	㮐¡£AGNbcu2FGL J1912.0+1609IVS B1909+161?îa×VÏ«¶? cý;»©?bF*ß
<É?}˜÷º?¨¾'ä¾Ü? ©*œä?ì0´?ºÍ†ä"Æy?q1ÐßdØ?}x¸ˆP%Ç?¾t5=ñʀ?¹ßD|þü?êޑlÎ?§ûà–Æ:?‹pnç&ì?…~•¿ìÖ?Âε
¨?¦ìœPýZ?íYéóE©Ð?•Äÿ¸'I
?Xq%ÜYnô?:9"
øƒ-?´ÎëÍþW?•›ŒÿP"\?êkSœ€)?¸åÙ~°
ÿ?l'N§ãa?hÁ†*ü?ÅànˆQ{P?¸¯ïƒuÃ?çI/óì?ǝy‹dÖ!?}»µZºÀ—?‹û¶Ý0Îþ?Ðöò(²Æ?Çàâ¥Éu?ç·Ï	¤ï?±ÙÀñºQ|?™oC
¿í-?'‰(†|žq?ÍòێJtÝ?°íç,R!?é˜tô|FÖ?­3'JëŒ?faZîÐ?Su	Òq¾h?ÉEÛ̙÷
?­
ÏG6±~AGN4FGL J1912.1-0803¿ï@T.‰À zµ^ñýßÀ8¬™p~îÀ;~^sRÞ@ƹ†sø@"òü~¹?­‰w¸sN?¯wûd9æV?ÿ–xbm@ËN¢$'–?ï.rýMž¿à$åýö:"¿ä—‹')»e¿ã½/
/¿è1ÞõCd¿å',)S¶`AGNbcu3FGL J1912.0-0804PMN J1912-0804?ïO2}ß1‡?‡U"S€ýä?@yè®ØÆ?3BÙ›ç?••áÊûó?†ûµç"¾S?îä°Üú ?¦	°2+Y?KŠöUÁ¯a?aüÕ§´ˆâ?¡FÓ!E?¥…¯ó?ï$x'9??Œè	[vÝÓ?n`Éý»0[?sF¡'ï–?—¤Ö{±®?Š¡¾ë³xÛ?ï€BËàg?lÃó¦}-?a=ï¨Ý—ë?D›(íïd?‹ŸÑ*ÐDC?jejÀ£«º?î;ïŒë5n?ž'¨Ш?PŽ&úËÀ?Cý¼Qðs?«¼•øôIÉ?žMügõ&?íHš+Ëñí?·p.í!'¼?Yù²¿¡?oFIæªû¶?µV֋[v?·68.ò;.?î"ôbÌÜ?˜RQ J|•?u¾ÉÐSJ?x‹d¦^€?¤åâ‡ó?–²ÿDŽèJ?îªb`°E?‹T¹jÅEÅ?yGٕ¿?d›¡êGS?¢0öÈßÎ?ˆƒA'»káAGN4FGL J1912.4-1222?âuš
)U±À$n9'ÈÅÀ9PŒAÀ;M¤Ú?|@'ñb~Š@®³Ý¾?¸×4ÀãÓ?ÌÎü|è³Þ@]žvx,@à'i¤‰b?찔[p¿×"¼uf´j¿ã"Àíp†¿çs¢¡¿çG8¤¿ïÿôA…ÜMAGNbcu3FGL J1912.6-1223TXS 1909-124?îð³wÍR??–Jö+<…?ŒäÌ,oÈÛ?‡¦ÁþÆ"?"w*é>›½?ŒðªVé?ëŽQR
ÂY?À´÷öØÿ?Š§}÷œ?˜æax‰â>?ÀBålj[?¾q?L4ü?í5bÛi?¢ J}p¦Ù?›6úSrâ®?•lÒB*èy?¯aÉqï?áÀ'a"¥?êØ)Ê~¾Í?—
Mœý?—â²ÑÉÃ?wpˆ5›Ì?Á»üÞU?"®
ûí²Ý?î¸x=9®?§NÒ|Z?•!wy'A	?•Pッ¾Í?¥c¼½§?¡TéX¢?è¿#3XA?Ç| `CrØ?œ°î'â?¡WQoj?Éq}'NÞ?Åó_՞F?êéAo?¯o¡x‹,?®,]Ø­"'?¢\FwÄÄ?»ú‡	
Á?¨LDLK?ãD
Á½,Ï?ªlNXŽÈ–?¯WŒXŠ"?•J'ã¨9"?Ռòùÿ'N?¨é9ªp¬eAGN4FGL J1912.4+3738?ïÿûìR¬©@(´¡ß¹8›À:š.$ÖyÀ<CLu#˜‹@›C×ñ1@LG䛬?Å´'åLJ†?·Þh«?ûU_]]©)?ÿ|Øm¿Ì?ïîõ üпâcåîy¿éûP£†'f¿ÞáÉÿ={¿ïÿ~›'?ïõ!¬ˆŠAGNfsrqTXS 1910+375?îƒNÚê­ï?©‡@J?'$OR"«?–éÚŸXº?žqÕU='^?¤·u,d9?íS'ú×Þ4?·ÍÊЁ	?'ùM}D ?'rçÙ«?°¥"Ë9àÞ?µ§ÁX›É?î%µE¾óh?–ØÒó
+Ü?"|oÑÄå?é®X8=n?£ãíh¸K?þӞçÐù?î rµÃà"?Š*k¹a‹?•ÛD}Á?yc³ûîÎ?£pçò³/?°yéPÀ%?온ÉÉsb?²¶ŽiuZ?ªë§ýaI"?¨‹å¿Ì"	?«‰Ëe+™Z?§÷Kæ^ò?胏EÓ?ÈbE"÷²î?¬b	…"<?²0å²ï"…?ÆÙ `PUa?ÅFÝGvê¡?ìsÖ"?£k?›Ï¾j?œ=<­º¡?'€¬óë?µXYÁ|˜?Ÿg~ˆT?éºx:4•o?¥븏ù?²N>¼f=Æ?™â¶¶8ub?¿Ýÿq‡#B?ž3LJÀÊAGN4FGL J1912.7-1250?˓vñ4FjÀ$ú#9ÀëîÀ:&êÏS)À;ÑÛ¤$é@ 
¿)öôi@BZƒU?ľªŠ­˜?±5ä¾[?ðãœ*Ù@oL¶çÞ ¿ïæó{??ïzOßK¿ådÂÝ_¿áà³~È¿äxgêŒÑ¿è…2ˆKAGNbcu1RXS J191251.7-124929?íæoþ,V?¦1	ƒÔŽÍ?cq@@~u?hО/ÙÌ?°0÷CÃÏ"?¥ÆE«"0–?ï]‡5¥©?›ôy­ý?OáM7ýå?X¿ù?â]?"PhÌÕÙ?›)ŽdtXH?íNj¼®"ô?œ«þµ±ˆ?€kåA½Ùx?uDÏËÙT"?¯lJç:ÿ^?šÌùŠžh±?íî"u©X?VØ)çû?}Ùq¦V…?[Á×
ñ›?­bªtQCf?6ò™[Ïh?ë@¥6°Á(?µ±{‡ÿ¡?us»2vë?nðÁ_2?ÂQÍK¼…Ç?µk£ÌHU?îs¯Îþïù?°X/¤¯ã?`²…Àøø?lÑA$UÕ?§¹ÚµKYx?°
ùiÄv?鿘
g&?°©o{Ö°?"­O?…²üR]?Æ¢"Àª»¼?¯j£Ïö°?ëw6©p?–ÁÝo,>À?FXÀ:·?w³·•iœ?Á¡X
÷Ô&?–>s	5SŒAGN4FGL J1913.0-8009?ïŸX1ªÀ;žêúµ=dÀ8ãÜEԉÀ;·%;ù«R@yiÓ®=k@±ƒÞFqÔ?«Îªžœ8?ÂWzzÅn	@§Òª\_@:Ë-?€{¶@ˆ¿ßÓ þ½¶¿åìÉ⌧™¿æáìï'{¿ê{÷"J¿ïÿrÁ¾{ÑAGNfsrq3FGL J1912.9-8008PKS 1903-80?ïÜ"E$Lf?aa>vÔ­?Y´á5g?P¡Ã76rå?gàŒ$?•?Y|:Ä
>å?ïæÑ>\Ã6?k-ÎÈ
'o?9B·Íxk?JúJ"QÓ?fj©G[¼?góØr"?ï£j'!¸? 
X;ßä?hž¿$@ò§?sú"ó%Ô?€ý«÷Fc?{x'ò"SW?ïãà¾ZL?Lº»§ǝ?BG0èËMÖ?*"OM†ç?gŽÈ]@<?IØàäo?ï¨}Ü8®?tö'Ü©Á1?kȱŒH?c×?ê–)T?}Ýg†Þ?n—oþT¬?ﶶ½¹+?ƒ4¶Càå?Qß¿{%P?jd¯š7?€>Ú^ÅX?€¦ŽãEÔ²?ïxÄc‹"r?‰"²9´¾?q0¿±~G?zûüL
?‰6‡D$f?"ÀJº6½Ä?ïµF㋢'?jvuÒeû?Z+º¨cà?H>Úf¾	©?~џ–Eº?h':ð)'ÝAGN4FGL J1913.2+0512¿æ™5‰W_ÁÀÊ›š$ÚÀ98
¢pÀ:ÕÈ­ç.@ÀŒL©ý@úo?Rü&?Êj»ìÕ¬?Ë­G`ç¡d@¥s!_Ì@KÿßÝ6?ïJ|€Y+À¿áU)' ¿éøn¦¦ÈV¿æ¼o»¿êě¥ãSø¿ïÿI)>¾AGNbcuTXS 1910+052?ÇkÔ
ïé?¸(¶"^?©#X$ÓJË?¡!Á:°E§?è"	"i?º® ì
º?Ü×@â&ý?ÂÞ@Mß8?¡–¡ï2æ"?™J§úø‡¥?àzõpLÿ?ÂcáÀ"E?×Iäò?²h'´¤Â*?»ª«ËÜs?¤àšq÷7[?áæ‹?²¾ž
Ç?Ӌ•ádo§?§'A?=í?²<"¸Ï¹?‡<š'Æyg?ãò¡\¨ïÅ?¨Ö89
`?½‹»¹ÃÊ^?­Î¡ö܈?©WémÅí?¡§]ˆŽ‡×?ê¹	ðÞhÅ?²ýwѦÎ?ÄÚÃæW"?¹Í½"4Þ.?©~¹§'¸?©²ð0=Û9?é170nC?¼Åƒåʓ?ÌßഓÏ?­)ÊAÁ¼/?½#Jz"¤?¦}%åTÉ?å#ÏõÈx?²/Ðó»¯?½4÷65z?›µe_Ò¹Ñ?·_b<}b@?"Ì•Y÷Ç?ét
²ÈY?£örjzOTHER4FGL J1913.4-3629?Ôðýsˆ¸ÌÀ3ÚªŸ{ZêÀ9³æ鮄ãÀ;'ŸJ³'@ë€nÐBM@$FE^¯?»ßð¯š?ÅÀüI'I@ˆ=ÿ?à@4¥/úĂ?Ѫƒ ÜD¿ä"²ªØ¿Ødñ†Ày¿ä'Ù‹÷ð¿èÈòýãñ¿êy
By!TAGNbcu3FGL J1913.5-3631PMN J1913-3630?ï©yÃæIK?Œÿ»õT¤t?s­Ñ°Éxe?|qžl«ê?w•Lrb,?€â'ôŒ?ï¾h« Ð?"Kd­h?Tw §'"?`o\Òu?{­é²A?'cÂåõÀ?îbº9Cºâ?™ë–ZÞ?†ï±ÿ?‡ {<	¼.?¤N°³¹?–JøÂaƒ?í¹À&?‹s)È°›?wU»
?ZIæ6(þ ?°¼¤.£§?Š³vW>?ïvoó?£ øP¼¹?°óō|ü?"Â*ŸuW™?€'U•mA?˜¢~JH?ï<Ôh'R½?—k§pWÎ?p-´Útw?w,›"??"Z*ùçM?"låԚF?íw!Ë	†Å?£>'ÏàYp?"ŒÕêô?ØwÛÖO?®ÇÕdr†µ? k-f.w?諉ÊÞ?§"­YÆ?•^RËÈ΍?ƒ[¦Òæº?ÊL÷ñÇ6?§N3äàSAGN4FGL J1913.9+4439?í;´î×,@-ó*k
•À:I¤¿g‰|À<t'Ç=@Ó@£%2g±?ÿJ£ý ª/?ºK_ú¼t?©æª!.×b?ðs
=Ö$@*fÅû?ïö Kºi¿éï=n¿ÒeÎÜŸC¿Ù÷½j.G¿ãV½¢…¿çT‰Y°u~AGNbll3FGL J1913.9+44412MASS J19140184+4438323?çåËv`"z?ÖÖù#dV?K}@¡° ü?Dˆ™ÞžÒ?Ð&ªrɏð?Öܞ³×)ê?W?¬é?‰Ö@À™Ë‰?WX~±2ÕÒ?a6$QàqÁ?…ïšZžVú?‡e–£>5?ïi'fø»?{'sU–Ä*?bÓº‡ê˜?_BNàŠF?s[Öæ7I?y?*ZÅ?ïHé@©q?n³Œ~çÞ>?týÝ%?Qâ˜Ú5¤Õ?'£`¨ódø?k•–aw/Š?é©Ô‰H'j?Òx¬Ï]
?a	Â9¦;?Vރ†
w?ɆÓKõ?҄ÇjbIv?îôøS/Ê?  
"U(?e{â&`Éè?q—‡œ)N?žÏ®'.~?ž½Ž[ñïü?îÀŠóþ-Ý?0vaÓ|?pq
¦Aˆº?i´w–d…ç?¡é/m¦­œ?ËG9ðÿ–?î+)Y{Ç?…Wz'öÊé?‰á®[Š'?nÕÀÊ¢?¦Õ-%þ?ƒWb«ðAGN4FGL J1915.3+1149¿âïáÙ?ö}*"=mÀ8vW0h}˜À:º|h0@љÅäPL@k9ýQÏÖ?Ã`qšL
?ÖFíD'o@¸0]•Ý@™Õ­œ¿ÔµŸ^ª…O?éO/]e¶¾¿æ	!ay—œ¿èy‰Ž‰›¿ïþ›{ñèæ¿ã¥ÁX¨8AGNbcuTXS 1913+115?"Àޗ?'ÿ,ûžŒí?ËV$D-"?Ňÿªçí?è‰Î=˜Åg?Ś¦rM­æ?žHÕ¢W…?Ÿ³»~§Ã?Ó¯>\;-?½ºÜ¿Ög?å6$³,'?¾
óYd±l?µ{6«Xuò?£'Áåï?ÑY¢OÃB?´kBøA?ä£Èæ@?´Ã÷ðʪ?–IRxU£·?zKêþ?Țg{JŠN?¢ÓÜ´Â&?é'O3o?¤4):?…`ܾÑDR?}Qû""T?ѽ†AçÅ»?Ƴ³˜•¯÷?æ˹k¾ar?Æý evãr?‹EB\V?7;"f¸?×ØO/Í?ŝ4R[Ü9?äþм+Ñ?Ån¸¶Pš³?ªíLü¶^?™dIKÌ?Ò>µé—™ö?¸ç[6"?å1Ð;[³?¹Øñaa?xÍH,EŠ?cÆ\vrªò?Î
R1ƒ¹;?°Rè(â'?èKÐãTE?°–sœ|AOTHER4FGL J1916.7-1516¿ï÷ØÒû¡2À(Èõ\)À9ÌѝìåqÀ;ÄSõJšX@#>¥ØW@oúcÞÍ?Ãû×ý,'?Ðô!ºåĕ@ð@|ÇÑ»@D]ÓG?ï¶A……¿áøŽâ[X¿éƒ†="	¿èTÒõ۹пë¨"HK¿ïû÷"IôAGNbcuPMN J1916-1519?ï®ðd+µ?Œ»B ^eÙ?giœH™û€?o`ïE&›?|Ó&ËIS¬?†Ú`3F~?ï}ëN~N?ŽÛŽ{]?b'ÜÓòW?uâ`Ǟð?ƒü2bÃ?‰Ó‡±L¯)?îK©‡ßn?Ÿf
kœ‡ë?påÜÝ?‹àN-[;?§ÒÛ"³±?š7£Sƒj?î÷¯²hP)?yˆ¡YÃt?wÁ'&w?X‹c£ûá¥?›©(À¯?x7‹õӔ…?ï; ;cI?¡óµbf¼?xnF×mKE?%Ÿ°4¿¾?'pfàØÊ? 	¸"ï[y?ï
†¼Oڑ?£"›õ<Î*?y7æàP?‰ßcHõM?˜.¼Â?žmº5¼?ì´ç8]ê?¥Y!+å/F?š3±H¼ü-?'Ì¶F?³Ò|rÃ÷#?¢¼É¡(—?ìrÃ>âœ?›ó;üyq?—ÒͯÛ+?€ ›k¬Ò?¶¨1Uƒ,T?™-ä}=AGN4FGL J1917.7-6442¿"•/®l°À;•»¾‡À;	ÏDvQ–À<ªJaÎ@÷\"ë'`@œ2?Ñãâ» ¨?ÕP–ñH­@=p£×
=@'ŽÇ®Û¿ïÿÇ*Ì\e?ïþΈ°=¿á%Óύd¿çòùℚ¿ßë,~Ž%r¿ï¿ü¥¬¨AGNbcuPMN J1917-6435?︗ '~•?sˆ4ë7Қ?WX¿pVñ?PFٞ.±i?}ÝÿÚ«.°?q+ ú%go?ï•g.H£ï?ˆ`?aãs'vý9?o©oÝ)©?†-W°rì?'F^H1µk?îÜQ Â¾è?"fð3‹?ƒDzυ‹?'È6ڙ~k?šÓÄ/;Ï0?OFPŽÏ?ï8ÏTLÅ?q8é1…©»?x¿ßï‹^?[Ñ þ'u?'èÖ®a•?oçå‹A]Š?ï3TÛò?ÃùeÆQ2?hqØޞž?^vš‰?Š.#jB‡ó?ñ­ m}?î¤àD×S?¤]!×Ùà?dŠ²5É?¹âu'¸¶?¡¾Of¼f?†ÃÆAW?î,Qz?™©vG°q?Z†À@Oæ?Š
þêX]?¥hL¬—Ra?"ƒ¢tO?íÿm²FIø?ŒòKS¾Ø"?ˆgî<8^y?y.Ü!ٍˆ?©ï)LHê?‹¹·µþAGN4FGL J1917.7-1921?ê.Ü2µ"ÑÀ,¥(IË%-À7õ"i†¬WÀ;jUõÕÛ@âÈހ©^?þšÈ:£j?šlûÅ¢zØ?˜\ÄÙ?üp'|F¢@:ŒÁnö?à­ÆÂqª¿Ò‰½#ã4¿à_Ðéſ۞üd¿ó ¿á5Мe&¿×èÔjOÿóAGNbll3FGL J1917.7-19211H 1914-194?ïë1Õ÷)(?WebÆis?&¼)­R·?Ýi.Ä?cbglA?V4š>?ïÛ¥QL'š?y'jhÛ¶ø?A6Û]°©?O"V¹?p{Ö£Wä?wÓû°\$?ï?Ƕëí'?'«ØF¹³ý?azsV–g?lÈ»1ý"µ?•×ººÇ(Ø?ðßÈõI:?ïuÊÐ{á€?p"Ø·¸#?f:ôCóm ?Lᝠ(?ŒþŽÞ!*j?l¿Â§Ÿ¶¨?ïË'¸¦3?p=^Ï\_?<'ª7ø€?3°24Žv?x¢ù`qäX?oëÂ}]å?金yý-N?Ÿ.–¿?VéÔÊ9 ?jδÂ`«p?"Ä=ÜUh?}¯HсÈ?îÙÐXzû?•êpî÷çO?aàGŠL"q?m€Òã'.A?¡Dõÿ%X?•Ö9ÌÄ-0?îñPÅ	?†Í_'oÒ?v{ÔYÚw?dcX¹Xg|?œ6ú³§ò)?";çüñNAGN4FGL J1917.7-6930?è ²ÕªÁàÀ;' hUSïÀ:NãF¶žÀ<p(ßó@Òë1¼»ˆ@SX"?½qõ:Õ?'Ç]~4Ê?Ô$ þè¨Ë@
0#	ÅP­?¡UMºHä¿ÛIÞ}¿äzï,D¿æ8}¿H€¿ãÈM Å¿Ñ×DÔñ4AGNbcuPMN J1916-6928?ïò:l¯Î?GL'Z>O‹?+†Ü9\ÔK?.é'*v%?Wn°&k×?Efrý]?ïíE,Ùô?e~4R0é?(¤šÆÕJ‡?9›¶ü#ã­?a0Š˜ Ì?c2‹7íb?ïºKþ†-V?n'õ҈Û'?SêÆÁo?Tea

%?}ßO:½#?l9i…æ—?ïíŸ/',a??àxY÷ä?12š'!4?SŠÚ7•t?`:Že˜¿	?>K­Üü?ïàYßé?d}y«":5??™Î‰~?4æ|Iˆ8?k²ç+œ]¾?c¬ÆÏ2.Þ?ïÃ=ŽÎ0ò?€"]
Â]?:Ã.AY<Ê?PÁbX©Ö?|µ´3žŸ?~x¹î¯f?µ\²w?º/)xö<?`¾Cååyû?a5Jݚ_?‹bŸ3ÙÄ?}OÛý'ß?ïÍcO}
>?]ZÀßdo7?F­T2?1LyÑ`Xþ?vŠ÷Œg²?\4Ø÷AGN4FGL J1918.1+3752?艊^N{@&à=ݱ ŸÀ:Â7n+VÆÀ<vÒõÛ¹Ð@ |ú<ü¶?þÓCßRáN?Åb}äzC?¿H‡h:&?ùf'•ù@sBdÔjü?ïùfˆË?ï³!å#¿Ð_¾+Ÿ@¿Ý0¥dSÉ¿äD-÷Š¹¿ÝfN=¥§ðAGNbcu3FGL J1918.0+37501RXS J191810.2+375315?ïцö²W?kw(\ñ?B%#oª?8÷åp,ñÏ?t÷á´I¢þ?iõïÇÜ0?ï|x»Axà?'ã´`hwB?W×'}?`]ÊH֎
?Ž(©a?ú§HÔL?ïkä]ÉE?"¢Â
œ©(?^ÛQ¦º	>?^Ã/‹$3?•¿,k¼é?ƒæKz²
Å?ïHÅ'€¼B?rÅÌΈb?wpCYÒ÷b?\E®¼ÍY?'J6ò?o?ÃXg?ï•$'º
?€L}¹–'?WÀ´Ë¯,‡?PJQ¬Gç?‡¾Ä¯5?"Þ
?ƒ]?§ýlƒ)ù?p1Vã´>d?8; ÀV?¤	›}RÚ?¦
&udÏñ?îÁçëÙ?•
L…H ?g(lJIý?c NDÖ¦š?¢o	½f¿?"[BÖEDÎ?î/S"Íñv? X8¿ÿ?Š!¶!ÿH?vœTâíäâ?¦'`K|ý˜?‰í74ü_WAGN4FGL J1918.2-4111?Ê£üóAgÀ6=cEI¶,À8^&åGÀ;wF'‹ˆ_@3,éŠ?üíy¾Ô?¢ð"½DC§?»œÝø©Ê@ãÔHµ{@ó8–õOx?±
9>æ¿Ø6êx´G¿Ú
Jk^ì¿ÙÖØ9¦ë¿äw^o¿ç;C£AGNbll3FGL J1918.2-4110PMN J1918-4111?ïß÷ÅQ‹ì?eÌvòw>?N½~Xƒ?TM¼âü†?hƒËyE?^²È°+®?ïƒÚì†aÀ?Šïق˜?lJkœMÙs?qàHŽ?‡ö©õDU¾?ŒÐTEñ^¤?ïQ›-ù:?"jEØ¢$?ƒ^{ȏ±§?ŒLŽƒMîD?ˆ:¸ýPçé?ˆ/xo{®?í¶Š~|:l?Œhn_v`™?…§l‹±‰?eûð͚>?¯-|÷ã¬?Š±nÜÞf?ïÇ#Cë«ú?q{4ÛÕ*v?U^ÙÕÿ?Q¬v?
è?w§uöv?mŸW—I?îÇאÜAñ? á¶¦#?"'Ac?"TÝÊB{G?œúÅCñ^?›³Tã?îÜ9{Ä?œí¿|%l+?‰N'kt?YŽ¡ò?—ш}¥bÊ?•›rϺĶ?ë}ˆÆ? ž»_š¢â?"<Å
ä{?yxb"ó¶?¿DÎŠ</? 58'ŠàAGN4FGL J1919.2+0618¿ä)ÞTC#À
!ÇÃx5À9wEšMôÀ:ö@&t@õøADÃÔ@ïOP ?Ù*æÞpä?ߋ:[E ô@	áZùJÚ@ÉIýúí¿Øí‡Â׀…¿àâeàÚuØ¿ê"¦žô:¿ïÿÚv»œ?ïøÍaO—¿Ï€™XG#AGNbcuLQAC 289+006?ÖøkUR[±?ÉO¹}'•?–
"º£Å?"/{ŽXØ?ãÓ]¯ªõY?É8wQ‰Ï?äa¼¥"«Ã?Ëà†ïY$ñ?ÅâúՁ?™kzý0Ê?Ö>]õ9äŽ?Êu匃¨ä?Ý	Á˜Cáµ?µUˆK'A?¾ê¼21Õ?©ð¦j¿9Ý?Û;[/Ú?µÒñw»ž2?éX|f`À?¹Êڑ'ýl?TQZeÿÅ?R|»Fxn?Êuk²*µ
?¹¾³	é?Ï
"¾6 ?¿R''^?™—)iʎ?–óöÖbW ?çp£($$?ÀÜnçz‰?Ø (O»?̳,è–?š‡+V:·F?§"ÓÔVn?ã¶'Ž?Ë&Âúä?Ò·úp b?²«~#•ˆ?Æ^ˆ‰Úgs?³Ýuӊº?á`ÑQò?·!SÑ}$ˆ?ßתâõ·?ǵ>27,?mº÷	þ°Æ?s[ÅX¦=¤?ßí†fóh?Æýt[,ݕMIXED4FGL J1921.3-1231?ï«ãÎq»À(|Ä&5ïÀ9þ‹‹¹ÝÀ;ÙQAK$@ìÀÜ©Ž¯@$'ÇÅ&?°€m"Ã#?°ö AÏ@0
ø'@ªÅÎÖ½?çÏó"
3`¿Ðÿˆá»q[¿âA:û¿Þžœ)¥ì¿á¿ï~Óo©¿äҌ)nŽSAGNbll3FGL J1921.2-1232TXS 1918-126?ïÄãÄW»?kÈԟpõi?LW2µ?>Vî"iu?z7œiL´?iIôïp1?²Šèb?‹™¨êÐW?aVÖ·˜n]?eÈۀ¸¯Ü?ˆ}£Y)ö?ˆ}ÆRªßÍ?îïú¼Ê ?þ]Gì™??qH'G?jÈú±"¾?Ê &}3?±m;eÞa?íé!î¬	x?ÁוnŒß?'(ä~dø?kN}ºÝ?¨YܦoÒ?|ç)'i4z?ïfgš[û?'ð­Øºô?hø¢~õ?[Sogl?0͑éƒ?€Ü›†³T?îÍÖê\¤?£b0"G7?u''ÃW²?€ž+Ü ? p_(M‰È?¡9¹¤¬?í~rbI? €;¨çY/?þ€‡ê?}ê	Ô)4o?±ÌŸ‹ü?žzËÕÛ_?ë@Ñ>K•*?˜_£ü	€{?¥P wñ^?…F÷¾Æ'c?»sNi?"ìË7#íAGN4FGL J1921.7+5817?¦,XnC9@3	‡¤¤—À;Ãú%Ëk¤À<õçoæAé@!×Û[/ür?ú}$ƒmj?ÐÃqnØ$ð?¼Óæ``º?ñ§Sçáv@öh@†-?ïÿÍ?¹Ss¿ïÿ'ÌÎzL?ïÿ°ï÷t@¿æ#Ã>-¸¿¹øk µW:¿áG»ëÓùAGNbcuWISEA J192158.68+581708.5?ìuPOE?ÁI8œîQœ?K¸Å‰zËm?O(—dûÞÁ?¼ õ<é§?Á@ü»c)+?î¹DoY?©òüBxx÷?uЉ*ƒr?|,v»Q/?¡±®•'©?©2[$œu?ìœ>µ¥òK?¨/Ki'G?eÛù!&ÞÂ?p+H [>e?ºo*‰…>2?¨|´"à>?îê0~ì?ƒ"ÉçoYb?S•ð ô"B?J݋yõ@£? ºMu'.?ƒa?DíOŽ?é¼­<ò?ú³i=J'?U-+ÄÃU¸?RÓµ+#?ÈâñO@¸Š?óYËų?í‡F@"w?¸¾ÑöF?},<‰G5Ï?‹D€ª¸ºl?±ó=rg¬?¸ZÁ>9§?êÂ*X)rü?¬×ÚvGsÌ?cÃÞ'ÁÒ?g‡ºx$<•?ĨJPJ	'?¬ÒLO»‰?즕K^Ö®?¤Õ£vlaá?`Öº
6Ý'?aè_°­È?ºDŸÓU¹+?¤¸Â¯¶"/AGN4FGL J1921.8-1607¿îšŸÅúíêÀ+¾¯«SÖAÀ9NjXŠÜÀ;¹ðál—@ )`^dL?û;=Žc?²c/¾ù>_?·m?Énžn@Ѭ€&+
@
ïß´tç?6ä•¿£Ó=@§¿ØÕD€ª³¿Ð*b{ö¿áa'Ú¿×IÅEïÎZAGNbll3FGL J1921.9-1607PMN J1921-1607?ï¿QÁ‹¡?ªy]r£•Ú? zIÔ~­?Òj½\g?Öãk:±»?ªz€ ds?ïÜwIãxá?ˆ¶"9t» ?>ÓîÉ¢s?L?åá·?o®8õžK?‡xKÁ˜Ç?ïŒcûtwn?}Û)ĺþ›?bixRE¡?h_KvjO]?ˆLÀKTÕ)?zßòª;,C?î]ÈÝÿÐ?Ì®ÃÇ~?h]‡rª?K}扟‡{?¥tQÅ÷Cä?DWfpY?ïìÛà]o¿?YįÆ!z?0†+*;?,#]ŸÙ?aZªc?W‡ðòxö?ï¢T÷^?ŽøϖÇ?R8«Þæ¸Û?a%â©·*Å?…#èng1€?Å8r§N?ïM'¯,º?‡çJsãôÔ?h˓(ö .?nó g4\Ë?"A—·Ý †?†%FŠ?ì¨ü¸o??˜Õ"ãƒ\?{lŸRM¥.?dåøš–{Ð?¹PHS0?˜[¼<§hIAGN4FGL J1922.2+2314?ì2~ZŠ @!0¾
í)À9Ò°@¥¾À;¶_ !¸@ ˆaV݁@x˜:	?Â^´Á=L'?½Zž\! ?ýEª~Ä+>@âw¯äà¿ï²xË'u?ïüá½tÀ¿á8&êþ¿ÛT÷=¹žó¿æUF˜¶›¿àjëø?AGNbcu3FGL J1922.2+2313MG2 J192213+2317?ëõ¤æîzá?±|pÐ,?iÈøñߧ?^ ׂ/µ?¿ŠÊ€¹›9?±Yv½?ë*§Ó©?º*ē‡ ?xÄl§Û=3?€ÚBx™D?'eûSë1?¹¢+Ó1Y®?ì@€%@}?¤À$Sä‡?‹šŠ¸Þ¶ã?ƒ[Ž/Óä?ºˆ­|ê%<?£lÔ¼Ó?ì@ü%@ü?7 Ðüy'?–RdE*c?s¬mh܋?¸c…¶bÓ	?‹>gã¡Í?èÉe¡ðU=?¹CÏèª?…£û҆¼?€=ó£}=?˂o9&oß?¸"ÀväÝ?äŠ"f9ùT?Ťï‹òÁ?´0Ѐ¬%?–ϱ¥Ý}?Õî­?·?Å/yÀ5e?æì«ôSé%?²…u{¾M"?¢´k8?Ë×PÈë?ÐL|ЋU?°÷\[ì'?çÓÞnµÀA?¡ñn«7?¨iÆ=³B?ŽaDõo±¨?ʖ´—÷®?¡eÄ;?"AGN4FGL J1922.5-7453?ìoD'ª®"À<#ædM‡À:Õçþ{À<fH;Øô"@ Xr…®€?ýA"d~.Ú?½î^Aÿª?°!a#±`
?ógû&|k‹@	™Ñ;Ü?æ|
A±ü¿ã¶Ã«»Û
¿â2§Ý!ž¿ÐJoD³8¿ãâ"i·S¿¿Õa8¿!œAGNbcu3FGL J1923.2-74521RXS J192244.1-74541?ïú#{Éé²?E?‰¾"U?Éвùr!?̂Z¢–?DØÖ0MÃ?DÂÉh ÜÈ?ï⯖A[¦?i¦óFû'W?4î;K§€?A÷W"<ß#?j²¢ƒ#?fèw‰_ á?ï¿');@?t\ÜkҔ>?PL´"¾Ðµ?Z®s'i9®?|`
O6æp?sT9²'?﬋9ëšT?_€S›*b?Voü¿''d?69˜†$ù?'1ÞÞE?^EHnÜg?ïö×ø|€??~Ñ©ä?'ˆ.ŊÃ#?­.ÆFßý?N¾Ñ£»¶?<Ø/çí×É?ï¢|»¬,Þ?"/4ÿn¾,?K:ïv Ïä?YÇñÐK4A?…­"1H*?'gæ×Û?ïŸc*ÝV?ukÌÏÍmg?S®ð!GnÆ?C|l/?…±Weˆ±?tÜj´Ó?ï#ÂÿæÌö?z<ãM©>p?kþ:`ð?UbÒª~»"?˜ܖ8?yr¶ëwÿAGN4FGL J1923.4-2503?çÉ½ßÛÀ1ÄþG™ÅÀ;w/âEÛÀ<£|§‹@"RßÛGcí?Ø©Ý3¢D?ô[D)$¼?ïÖų,é@X> N¿@`̇­ˆå¿æ¿ŽU˜¸É?ï"Fj^¿á/ÿ¢/?ɅsFô†$?Ætð'^"‹¿é0…;=ÄAGNbcu1RXS J192325.9-250228?ïš_·ËˆÕ?Bcàå?USŹÚð
?J ÀÈ??†½™[¹Â·?€¬‹‹OY#?ïKóYº—§?±y°›?\nܗF3e?róƐ†?"º§øWß?±Nµ":ÎÍ?î3v—‡ç?š¯#&rF?ƒŽµgcè?†'ÿ;¾?§äé2ºæ'?•ÝB¥fãV?îˆ*"Š»Ó?—V}âšC­?3S\;¯?@o/Üák?§V¶™O^ò?—e(&Nn.?ïD<ò½?ûs©EH?p9Û
mSþ?gùXÊ 8?"nA³øi?ª '5Å?îë4•D0˜?°'d…S?z²ªp,<? ^_'ÔÜÐ?›ì¸+=?¨½DSÂ?íºA-á~y? ^tvì¾?;Þ)¢Úñ?ƒÐ)‡Óë?°zÌoœÕ?•"?폰¥ààç?¬ë¯åÒ?'¹RÒÌ	?QÚêCžÃ?³vžGŠJu?¬éé˜ÿAGN4FGL J1923.5-2104¿¹8PtJ/À0>îؐOnÀ8¡Ïi_?+À;¨''ûÈc@øÄI¦@	<Ú{áù?¥òÀ§Oµ?ÁÒw[¬#4@ù&âÂØW@0—d54?œ!¿Ýø¢¹ì¿ã×Tæb¿ãÓ?ãDÞV¿êüí@àšà¿ê«hÎör¹AGNfsrq3FGL J1923.5-2104TXS 1920-211?ᅡl+wR?oo{ë`D9?fJó;r/?_ï\' éQ?uPF\
c?fYS
Å}?ïí&/Oßø?g¨¹Yiß?1×Q—ÃœË?E$N­í9ö?`žæ}'"?e®¿¥Ú¶?î¯_àÕF?œK'ûoÍm?—L©+&C?"~ƒ3hǜ?'ÇZ¿`Ÿõ?jU«¥'(?ïöõ>IÖ}?8´|øù^?éjNŽD?	Æë9}×?Pvñx¦£y?6Ý2d÷G?ï{t™É®ú?ƒ±)ÃÉÊ?vagötÁ?r·ìkO»ž?…ò%'ã£?|Á6†ÆÎq?ïнçÎþ"?€ãŒ`ÜÉ?PÁþL¶7?rÌïÑ\?spÆeüEx?zPf5CL¿?í¾Ú[ß,~?¢µë'hU‡?¥؊á"?œÿ"ZN?ålŸz)?•9àF]N¾?ïéØØô£?W@Hn}'ô?0$)þʬ|?#Ñۂÿè¾?dÝ¡ò0Ç?V,"‰tçAGN4FGL J1924.2-1549¿ïï"îJÀ,†)Ø@žVÀ:õ™ÊARÀ<EÏ¢j"´@ È¿èbÕb@`b
·'?țëƒq9(?—;ƒ8Ú.?Ó ™?׆@k¨÷/¡Ù?ïµ;K/©;¿ì'Ë $c?ÞQmü÷¿ê7‰Úõ¿œÚ»ç'
¿àõ¶€Z-sAGNbcuTXS 1921-159?îã×3"=J?§M~'ǯ?J{ä½&?G
È-=i?¡X8Ö"p?§:@˧?ïLà¾ú¯½?¤¼®è"x?bñ@2î¿d?lGºnÍ$?"Àäv'?£¡aÔ¥A?î—$êp Ï?'êRĝÿ/?dêjë¦ï¨?bk'"ѱ¡?¥?
¬×9?'s‹¡Î?îq¼H£»d?‰}wdzç?IçÑSý՚?@NõPxe?¨|œ1?§?‰jÍlå?íľ1Ã5c?«ÍìŽ\oZ?\s6YáyS?RK©œÕ?±hA–z	Ä?«'lÿ‡µ?îy—¿¬?µßþöpÒ?f…Ìò°Ô?z{{cˆŽ?¦þ'Q—f'?µSçRœöj?ì'8õ?Ñ?¤<c#y"?uú3ÔÃ?rŸIÀ>"=?º8²'H?£Û¤DÝŽ?ë Ú2»éü?¦u®7H\?^ÿö5?\ÛÙs9»?Ã?—3|ú?¦•­K´&AGN4FGL J1924.3-5458¿ïáԤÀ:"œT]À;OÖNUÎÀ<Ãü7ôc@ I£ÿyw?äԌê^®?Ú|"zÔ1›?‡ça@9ÞýPù@'²¶v??àbñNŒU¿×AV¨¿ê\vXKñp?ևáá1à¿èâ¬K¿ïþ Eð¥AGNbcuPMN J1924-5457?ï~lcøÅF?†uAn¶÷5?]¤lbªS?Wâ¥+¿¼?Œ°YhjçC?…efzø¨?îù¸?¢UýàÜr^?ƒ"‰ªÌ¼n?"( '4?—º›œÔ?™ €0ÅxM?î5pEž€ð?šÜÈ=R
A?ŽûÒùÖ}ø?ŽgþŠí«Ö?¤êëíy?•ïyõåIñ?ì	Å|)#î?§¬¸zóJÂ?ˆäªuE7©?"ØùØ}î?¼•>Ò3û?§Y¯£óÅ?ï=Œëã|?'‡ÍþËÙz?s+4¾x¡?o_‡ø?"ƒ'ÓoÙK?åN?ír{*¡Fë?¶u/¤ÂÉg?•$4G\6?¥æÑ¡Ö|?®F30¨=?°Øò"†b'?íoxúko?¡IêRñHë?"Íٍ©¼?'Â÷r#F?¯!ƒ™ŽB4?€•š9/T?é²G:|(?ºŽT—p?Œ(QgX?•2 Àh0-?ɧ²ýÔè¶?º	lª%AGN4FGL J1924.8-2914¿ïâ]íúxÀ3›ûz_A¯À8ªX-¾À;×/¸ToÄ@ú';‡@ò\f2d?¡¯Šœ¦"T? ¤!²Ø/?ø.8øo@‰ê¾ÒŽ¿À–—Ü€¿â‹…Û¿æþA¹Þ³¿ã8î~Mbß¿åÙv0¿ê$-ÁÚ*ƒAGNfsrq3FGL J1924.8-2914PKS B1921-293?ïô9úÝ?SC»ã返?&~Lˆžå?0ÿSWÐñ?T¾&…<¢Ã?PӎËõãM?ïï(çLLV?cÚôgLi?($o÷I?6ÿóOÆ?^­ì±Ÿlé?aJÆjb•f?ïoª¬]ä?‹œsÓ1Kð?iŽëºÖ"¡?wÇ»æXS?«š^KËí?‡.T†G¶?ï÷œKµi?7¾TÖ¶¾Þ?#"Ž+éÁ\?
öå
?LÇ9º¡ç?5›¶êi´?ïæ!Ãý¤?_UT}S:?3Þ¥²ÌaE?'4ý%@¿€?gs	gÕ͸?^++rŒžæ?ïÎؙoäP?]ðÁ^²¥?@âhY›?ZÌË0›E?v'·
e¬?€Ÿ"ð¥L?ï¤õ±?"$'g"e?k©òŒŒÜ@?s—ˆZ÷"F?šV"õ™å?'sWwv‰?ïëàXšËÉ?V	EC?;;án]P?1MœgØÑ?`¸+">(?SC±P\žBAGN4FGL J1925.0+2815?à-OJ"ÍI@AS½vdÀ9œIlÊ.À;þ)ÊÔ¥@ W)HΦ?ÿW¹Ëh?´øá.-»?¤ý"ãél?òÛHZ⤥@C ,pKm?ïÿ"å­nc¿Î‡ rÑ®´¿äOÉkï<¿ÔrÔ§7¿Üø°WK@¿âÁ6á¾vsAGNbcu3FGL J1924.9+2817NVSS J192502+281542?íà'-ëÔ?že8Xn&?e³‰¾0?Wî̐4À¥?°Q*ÉÒþ\?²0L©™?ëà1àðÃ?´ø«ÍΪ?p¾ñ"÷|ø?u¨¢s¤?¿òß‹Û?³VRéy.T?íàg‰Ú'f?•¥øEÎÆ?~¨™ðä$ž?smÏÅßJŽ?®$t'¿îŠ?"0Mfzï?îÄR»õË?~YÔ¶ë?ˆ"boƒ=?bù_OåQC?¨>¢4ð8?{šd¿Ð™?ë"-iš£Z?±ªpƒÕs?{¤ö™'?nr-'­â?š*+UKê?±vOm1£ê?æ4+`€ô1?Ãí@é1åß?}¯G¢%?‡ç¯`²?Ó ìý¢`E?ÃcŸTÍy?êËí!?¨½
°.ÇÄ?¢Ú͇?€Så° }®?ÂùېVqH?§öþð"¡Ç?ë2AI‡™£?–Îm€­? M¢Õ¼ç?'nÐÂvš?¾G&ã¢.ò?•0S _2JAGN4FGL J1925.1-3358¿¹™›ïužÀ5H¹ý½/¡À:qè«O¥À<‡çÀn@Ôíè¦G'@ԏ¿%D]?Õmfr{?ÒãízÂ=þ@lû%¥«÷@•POù'~¿ÆIà‰B3¿ém2}«§c¿àê^u׿ïü?OQ¿Ï‹Å›€$¿ï©$Q ˆAGNfsrqPKS 1921-341?ï±Øê‰Ã…?~ Z$Ï?Aå
?2zJ?>g^»œÐà?'kt¨«}Å?|èfÃì*?ﱔº·¡l?"0AÝä*ñ?[覇Á¦?hö–Ïc\?€¼‡dø¥?€tŸùRçW?íéÕõя?›³•OOL?"®ž¦ƒ=á?ƒÜÔ݊…»?¬6øùF??š{ê&çÚÌ?ïn'Oû?ozgï–é?C熃vÛ?0¦7Ž%‡?Žåý°`¨?n¯{ZJÂ?îÞ×å•×©?¡G¥©Cñ÷?Y\2OBfb?W
Y *'?¡G žGµ? Öiû
«N?ïêµ·)?Ÿ–Ž¸š.Î?s
Â(Ô?€ýŸ¯³Žo?™Ÿ8Þу¬?™§)É,M?ìQb·ôè?¨ö
VÎS?gò‹*ô~?‹vXŽñѽ?»ÛxGu›Ÿ?§Mtþ´ÅR?î"9B–Ól?Œ€ï"5?Q·s­¢i:?Gëö‹Ü*?¦.°;£my?ŒA'ˆGFAGN4FGL J1925.1-1019¿åL5³@3ÍÀ(@^_0çÿÀ9"¸:n×À;†¸›½`H@Ì®EM<@Ò<B¦m½?Á†Ë¡(¯!?½lvìÚ^@`GMœk@¯Ôà—"ì¿Ùû/€÷e?ílkûѝ¿Úö` Éd¿ã,'Ž2]J¿æ>o;÷ýÓ¿í0¯_Ô{îAGNbll1FGL J1925.1-1018PMN J1925-1018?ìs Íij=?¼Ñ'ľ5…?qBuáҚ?t]Ãærê?»Vhût´?»åOºþC<?îiŸo,ÄÀ?§(÷¸6Q?'§3gîS?—†ÿg%? oXÓUÓ? ¹ú¾öÀÿ?猨ÿàlß?°š¡©Îê
?™wÁóG8?‹ð‰8¥d?Ξx	À·Ú?°¶RRÈ?æø&²ò?ŸÍʉ⨒?°\J{ÊÔ?‡ÍЭ]ð?Ïeúi×ÎÍ?œFE²ÝP?êEM"Å?Â7`Ýn
W?Š¢kHz"?‰Ð]rnSè?Æ. ¤»5Ì?Á{tD?ëÈß¾X|?½;õ¨ÒáS?¬l"<mõ?³UÖí$@?³'½Šêž'?²´9eH?áãíÏ(i?µ~ïë:1?¥'ò›¾aû?"Û¡Dìj¸?مæ
ær?´Ñ9³0í©?Þ·7J€=?¦3ezþÛ?»m®wTÓÊ?šØ,­Ý›?Û
Ý*àJÐ?¥h	'xAGN4FGL J1925.7+1227¿æs·8L2ð¿ü†«pÀ9á²7QÀ:È[;ù@¸žÅÓ^a@§;ãÛÝ?¾TÂ(Y?ǸMú3ã1@ïƒæ©í¥@ë9Û׿ÁÙ}µ7"Ò¿á¡Î¡¹"Ì¿ãȑûž¿åªÆÇ©¿ê|=2v¿æÍÉ¡õÔAGNbcu3FGL J1925.7+1228TXS 1923+123?ê‰-︛N?Âü{4Ãoñ? À±ý¼Ïl?°sí]àÆ?Á«ÂSL-?Àçn†õ?èøö˜Å?ʙ/ØF
è?m=Hܤó?{r «\"Ê?ÏÏ0»oé?ÊE9Ôüµâ?å"iêTr?´LCßl¦`?®.,ŒÄ? â17*o²?Ñõk%³Ž?²Ï\0°³?éîlUÂL?£íkÐIQ?pùÙ(Z|?Uk©0ºVÙ?Ǿ)$*q?£®µóxz?éÁ¢bH¨?¸½«â:€?Ÿ3Ýeôò?˜|¥u£xÉ?ÅúÊr:Á?¶#vp?p=?㽊˱«?ËÿaóBµæ?pJ2~bË?t3Ž;±?Ùµ\™Å¿?ËÀ(,L—¼?äñWø~ED?´JVl´Ž\?°Ã^!?Ÿå\Ü<?ÒŸ6ÖD´?²×K‰ñ³?âM†ˆµ?´Ù&:ÓðÀ?…Æ'³?q֓´K c?Ú¼5Ÿbö?´Ä»IV[
AGN4FGL J1925.8-2220¿ìlS€ÁÃÀ1?´åOz'À;GoçïhÀ<ˆÇ:¼"p@"!ëu(?û¦Ô€u?ÎMoÊhC‹?³¹? Só?笇²çHy@'Eã-¿ïö^½|?ï±Oޏ—ã¿à]LÁú‹Í¿Âï,ÉÍ¿â¢y|¿ªYÆ<\I$AGNbllTXS 1922-224?ïÀ†D¨&?'ólZ]?&'"$PŠ´?XÀiD;?A°TÁ*\?'ñðnk7?ï°¼1¸Î'?†ðÕæ]	?N'u‹i/?X0	î p—?î|;(?…vo6ÞRJ?ïr©£°|h?{[fȈ†?WçDÿUÃ?Bx©[ñÔ×?,WFÄÒ±?zë،cÈ?îªÌ>Sð?ƒúÿ1CYõ?gا­Í½ì?Q\à•0?£Õ±ž"K:?ƒ‰Z?½3j?ï¼HÕÆ^?t
Ò¨­?3#Õê‹ÀÍ?%©ŒuzÅ?€T¬ÂÖY?s¨ý~â.?ïN"uWê?›yĕ…]®?`z ÉIn?vœ²Â!Z"?","²T•?™e&æÂÃê?ïÇ+Î?ˆ(Ðuýð?a	0ëÜ7É?^«ÿ}ô)?š¥ôf†×&?‡ˆ`â¶?ì4;KZœY?ŸvÛynô?{*ÎmˆZ?mó>¡\xÕ?¼«xºâûŸ?Ÿ¶Ní41œAGN4FGL J1926.1+2059?Þ^ìD®±@v]¤öÄîÀ9†V›HÀ:÷¶‡æê@Ð"—¯Š@ž9ÛT?ǟ¬ƒ+C%?½Ùß‹?øB;ëh™?÷ž§ªÿH?î+h~nšè¿äIî*ëf¿æWð}ðÇ¿åâK^Τ¿ï°Ö+ñ'¿ïý,ÆAGNbllOV 239.7?Ò±Èâ(öç?Ä{.£Æ2?‰"ĵª…ö?­›b~F?æ@Ì|"˜å?ĦºÃ¤žÊ?×hö¾?Ȇá±
y?¶'Ï×oó@?®Êë"œ?á©qûä?ǤB¬šIº?ظº˜î?³Ì¹×|©?²Ú=‰ßx‡? °0®Ð`Ì?áH·ñÀÄx?´(µÏÝ?Í‹•cù?¢²FÓgà?»Õâ¾.W	?"ÿR:r]9?å= ÂáD1?¤ÏfLh¢ü?Â	Š™Ý?²ºœï³ƒZ?~jòšÅF?…¶<×:¨·?êùËú??³­È‰Gò?Âc]ÖAb?Àjt—Ep;?»æè—X¡­?·»'ÒÃ	i?çê[•ë?ÃaÔoÈ)?ÍÝ•º'â?®DKèÄv¨?³eq[¤ü? ŸRààp'?æ̸]ˆ?±`sÇȸ?µUÓ¨%|?•9
ð¦?Á$¹ó¬4§?¢dÒG1 ?éÆÈÉ)w?¦įûclOTHER4FGL J1926.8+6154?âý˜¸"Qš@3¾š^»w:À9ñ\Ï
ðÀ;Îm=ðüW@Ã@7ü?üŒ•¿ðEx?¬« Ðg?µÜÃdïû@|XƒNÔy@>C">™C¿ã`䡪µ ¿¿öÔ]9ìá¿ÜðÄ£ÉH¿Ør/ÈD§Ð¿Ûwp#ÿc£¿ãZã±àbAGNbll3FGL J1926.8+615487GB 192614.4+614823?ï÷‡†¸m?B?-u'°Ã?+bŠ×òÔ? ¯¿Ùܪ?K	DûDGð??¦û ^Ž?ï×û$?tÄ+Þ-?NW%Û Â?^¬¸Ç]?p±›­­9?o±2‡"³Þ?ï´>fÿ#È?r/EÊ-ðÝ?_¶ÓCóè?e¥ƒÏ"?q?}󐝣?l†?ïp¯ï¶¦?g5hy_>?`uŠæŒ]9?@ þö­™¹?¶¡e‹!?e~ÌÓ¥h?ïñeÁáóa?S›–Ñšº?9)59&dw?3­õ¹W,?Vê/EFu?POÌ»–ÙË?ïÌVnz?ˆG·,Z.¨?`©B'ÓQ?lµ·«×"?‡¢š
 ¾«?"ºñèl
æ?Vx˜Ô?y™Ša䒹?c 1"•Ýn?hâUõ¨×±?…ˆ]ø|՞?vÇ,¦†z?î«TCÆu½?ƒ«öuã?r^]Eµª?Za(jE×?¢þø´€Q~?ƒpÂlAGN4FGL J1927.5+6117?ª‹:!&P@3qí9SÞ¤À9d²<'ÎÀ;îQ°Ì¼@s7ævA%@ÞÄK?¬l«`&Âs?³"ÁO"ç@+
=²é@
¸`Ú
x?ï÷náàb¿Û&¢+8'ï¿á½< —¥#¿ã;©p¨¿ä{`H•¿â¢^d9eAGNbll3FGL J1927.7+6118S4 1926+61?￁CÑ)í?±©N#ýË?U~}t –?…º7È?zß¾©4øs?®\NiØQ?ïÇM¤Œ£?{Ïý	Ôµ¼?Y,RöÊZ­?gÁÝ©ín?v]ó"®?tFÙ.>Ñ?ï¬í^›I?oò&aŠQÝ?`ßúåۄÕ?`Và`w>ô?€ÀEá#Ü?ik:
½É$?ï!FӒÓq?l6B5rfD?yÃ|CØÔæ?SĞ)r&z?•fF{§zµ?gÿT[dfD?ïÊß-2ÏF?
NºP²ñ?U&ѽ'ê?o¾ƒêu÷?uFµ»öù?ˆßáèÂë…?ï_¥,¨]4?"×Ü`î#?n$2Zlã?yyª5%*L?FÔCÏÛ?8(í2?ïp	™B
?'4‰ښ•?pŽ¶%fM?tÏÂ8´Ó?‹¶>'xBP?z%
b1?í©àž2R?ˆÀÁ²¯˜ž?'˜äW}Ì?qƒ˜pbµJ?¬•ë(kÛ?…wg8ËAGN4FGL J1929.4+6146?â~rµV`@3gag#$ÈÀ:t+'~B%À<'z@¬Þoâf@$&5îþ?ώÜð±X?ÃÁ• ¹?úNêHޖ@}}¸'ƒ%?ë™.9Ï/¿ÝÖUa±Jæ¿èÚò)}¨¿Út°`Ûb¿íޥœÈ"¿ïÿ±@LAGNbllTXS 1928+616?êY€ò®³²?¹9¤`ãi?¤a)|ÛZË?Í_¼%Ï?Á±ÕimF?µ@ºâíà?î#H²eÃ?¤°3~¦†ä?–i@üÌ<?•»wÖIyü?¢–ÞÂ,Z³?žîf<¯d°?ì¿Rv£S?¢FGæ]<}?˜*ïÒ<L?Ž‡ÔÑý.?´¤¿èbÕ?ŸHîq½Q?êVYå	ë¢?•«PRF·?¨¤qq®Ú?…ŒOõ"Ó™?À'oNŸþÁ?'¯Òxpw?ç ÔøÚ
½?¾uÿì_?±¶Š—? éFÖÒU?ÊüPÕÒÒB?»8ØIé¿?ëDyéÈRŒ?¸Ç.¡TÙ3?¬b—»l)?«å¸øÈc?·« 滜Š?°µ*NöÏ?éÔ?­Nùo9–?©)DŸ
k?š;QÅ—Ô?Å«¯¨œ
_?¨'Ñiij±?ãNæÖÊbË?§œ¢]nU?¸îívy?¡q
tÇ(þ?Ó&vôu«?¦ªÊÔÆAGN4FGL J1930.3+0911¿™»£žoÀSÛ]‰HÀ9)êFZWdÀ;ñ`®—@qÇO_c¾@8þžÖð<?ʋ ÆÒ?ÕC!ór@Êôj ‡Ê@8ú0³&3¿ëœA^ïúy?îâþgy‹Ý¿ëyIbI¡4¿èÑ[§Æƒ¿ïû•!ººÑ¿Ö‹N<Îè[AGNbcuNVSS J193016+091037?àÆnmŠ¶Â?ɾ2¤±¿o?Àæl	'N"?¾ÀêË?Õÿí )k3?ÇV'@•$?י|šý"?ÊÀ0º»…Û?ÃÝãËkù£?½)údà\?Þwõ¯š?ÅüUpÊÃ]?ÛljY¹"?µ4--?½Þ$°ZóŽ?¥ú%
%É?ÜÀíyUÚ?µŠÈgX?àœ ªãv?¦Â»ß'5ø?Éæ"iÌê? ðÃ8XÉá?ÑÓtô@%¬?¡¥²Ÿ†P?×B<Nÿ†L?Äus—t?ÊõU·Ây?ÅëÆ+ÀE?ÛCÕ<í?Å|õã¶7#?Ç=º¸D¡è?Ävu»v–¾?Ì8@~³˜?ÅéNýWóÌ?ã"QÏ* ?Ëq—Ø?ÐUCÔl1?² ¹ —‡?Âzõ½Í?«wʹb'?ã6¡2¦V¨?¶"bùσC?ÎKH¨»K?¦Ð¤€yùE?ÖzY¾Ée?±ãA»›¨ç?ڂ€œâ=;?°vjÃiâøMIXED4FGL J1931.1+0937¿Þ¸©‡Ö×À0É°·À8=éˆÅ6À;2'î"­y@ ]ꟸ?ûfÙRí
?ª­NWPôº?¸OÂ5<g@Fß?–@ò…-H?è#qߖS¿çè| åhO¿×ùÎøö÷C¿Õ¿r¼`¿Ún?¿ÜaˆE´?7AGNbll3FGL J1931.1+0937RX J1931.1+0937?ïʑÌÏ.¯?oÙÀX#ÈQ?@rðöþÛ??;Ó3F?x¨»Œ'Õ÷?nh~7ùš?îÓ§\zÕ?³·uªT'x?J˜V)µia?Yy=K—…|?®hd5';µ?³—:\æ?íð½-ƒ­? 4¶Ê?‹¶\œí?œ0Å9?ª¬_¢…"?›|qcÇ/?íÙ†+Â?‹6®OϚ3?fÚ
a™Ka?GîSۈÍ?°‡wý?ŠÉÁ»²ÚD?ïK•æÂÓ?' %r«?EÈm7¼š?@®ˆÉ?Š"§
r)?uªk>ãy?ê\}Fê?ÃZ":{–?^$‰<­ò?r½Ú€'xI?ÆSiÖÕ±š?ÃLÒÎeöv?ì¬ü@"?¥*i9¡«?'Ëxݾ?'j'z¥)ô?¶7«5Iú$?£¤
¿TFÝ?ëJOî!?£Ó•Ÿ×#Ò?x<Èÿ~ù?byN¬%¯\?Ãì"¸"?£•9XSb¯AGN4FGL J1931.3-1556¿åƒEßÀ/¾PÅë1<À;u–²^Œ}À<Ú.Íû¡@ "´+?û=\ÿµW?Ù6¬Ï×CH?ëpý
':@¹ÿ]BÑ6?ÿ¨C0¬E¿í"½«;X¿êº¬(©l?ïó€`°?¦°×½…uå¿íxa"·¿Õìò\(téAGNbcuPMN J1931-1558?ìæÈÁàþ?°Mª!Q?"¨¿²"?‰Ó›×S½?³ŸŠ0†_Ê?­P'	?í÷ÒßáR?¹ó;vx­;?¦Ž¥4"—?³.nÇ@Ã?§²o1ÚJ?ª`fiÚ–?êDa¡Z®!?¬'tƒló?«n@L\‹?›˜ú¬;Ú7?À÷«•?¨XÊ·íÄ?ê9'¼¢!?¤+KFeÅ?¨Åø™Å"'?–=«µ"?Àèvæ*/Ã?¡¦¶ 
ˆ?ëC$öb%?´ÓdBT Y?£«`kz¢^?šµE¾óg¹?¹@6¢!ª)?±æ+Fxù?èå[Úié?É<ˆ©v?½"¨r5¸°?ÂÊÊQ†c?»²x¼îø
?¼‰»ÑY?çÑçþ¹Ñ?´ó¾x•ß?°9 >1:¡?¡ŸÝΤS·?ț"Ë4­m?²¿õL=ˆ[?ã=?¢']?·AaµË?¸Ý"üÌrI?²ïĝ6-Ð?ÓN9Qšõ?¶‹8e\AGN4FGL J1933.2-4539?á¡ÞÊPE¾À:	¥e¶šÀ9Ð]ÿ—¸À<3Ð$ër@'.ϏÐ@Ïf"‹?·èÞü$SF?©¦>(ëÃ?íÀ‰þ#r@
ìª``ö¿Í…ÁµíbD¿å¬°Í'Åj¿ç³:¿ïn¸¿åíLŸ¿ì¬•à–¿ïúï,DAGNfsrq3FGL J1932.6-4537PKS 1929-457?ïóæ Í.`?L±Ø»±có?4&çE­?#¼k©*¸?S)›5?I¿Ìë·?ïåþ€4T?nyÍHý?7t<ªSj?DÉôŒµ9S?gøì'?jk®5pAâ?ïÇ(Ú®{˜?p<â{¹?Uƒc?÷?TŸ¬jF?w&ñÚðöQ?k>*˜@é?ïãϧPD?Hó0‡»·5?Lܚ"¾Ž?/®DHþ'?eÛùg>æ`?D»‹|{ç?ïèá÷›?]·Rú:NŸ?ChWHÁÚ?9°rIõ	 ?c
9°àé?YOPÖuWÇ?ï®û0•ý‹?"áA4Ân?H¤r¯qû?WÌúw³sh?'¶ì±Ɯ?ƒB°£Ô4?'Ãê?y¹? Só?`)°¦o º?[*¹˜æ¶ñ?"
ΫdiV?x#€ñS«(?ïµ Ø+"r?hsØX]ò?dËJ
w?Pƒì&.À?{n.O_S?cmÀÒNAGN4FGL J1933.3+0726?íxî ï†ÀM;€ßŽpÀ9!UŠv(À;½=1¹¶p@ ß6<ýâD?ü`¬}¡ìN?±4è%ü¿?­M	âÆ£?þ(³}pn@ì{"`'?ïÿÄ;-Óx¿èkþ‹‹¹Ý¿Ú®(ýân¿ÔpŸÌä¿Þ¾"¯<C¿Ùyª	bAGNbll3FGL J1933.4+07271RXS J193320.3+072616?í‰=Å¢$ò?¬þ«2œ€?P^f?}È?F¡mIº?³t˜;ø3?¬ÛÞ5öt ?ëüî	!Uª?µºM™;?^£FJ¢õ"?eöWáÔ×?¿ž›!^?´¼`ÎË?íŠý¡0´?Ÿ¥p"¸øÁ?tJ^Jq"ð?rs¹µÁ¶û?²cqÖ#f ?ž ¥iQ??퐍Ësö?‡¬s»är0?'ãßíÌ°Í?`¥V§Þ¬?±¨?†Ût\'±?굛K†¢W?ºb%›èJÏ?aȊå£Á?ZC~>#C'?Äâp¥&&?ºBnjfÄ?åki#@]$?ÇC"ï#?leúœ?}@I•ûøZ?ÔðaÄb'i?Ç$ã;pÙ?ë"ThÞ?©á8íô\?'Ò!a'ÞŽ?~–æ[Ë&?Â̐šu]?©u}°…?ê)¶\,&?ŸØ3ᘆ«?•È¬~9?zv¼ûúß?Ä ÿmD?ŸmN."'AGN4FGL J1933.9-1025¿ïüÃ~*¹xÀ,;}æOUÀ:™Á•a%µÀ;¼,k˜Õ@VK˅yý@Û{Òv?»4‹"'Å¿º¦ƒŒçÚo@Aâ"Ÿ@†Õ/ò¶ì¿Í™—@MøÜ¿éoÜfÃË¿í—Ù¥ù#m¿Ö
‡­ÞÊü¿¥K鞥Ù)¿ïÿ•ÂûAGNbcuNVSS J193349-102530?çAX€ÛÃÇ?ËOÿ‰YýÅ?Õ9,Bem?‡XËÕV½?Ðî¥5jVF?ËMM¬‹?ï6ŸÌ?©Ab'hÊ?k'KYÒ§«?wªÝ\éšK?•»½éyØ?§ÉfÒ!>w?é'çb>'r?¯©ßÙa35?‰¹´ü}gÕ?ŠÜ:eòò'?ÈÇ'­;?®p˜àµW¨?íÌNӀMÌ?— ËYö^?OxÑ2«Á$?D"»áU?±^—À˜Õ?–ך:';ö?á°?Q4â?Ï9úf|Ðz?ŠÙï<fÍ?ŸÛßêTÕÂ?ÚÆÓ¾Ùo?Ϊ‡ÙäÉ?î}^[!†?´¡=Žín?"Mͨ*?¦Ñï·¸‡~?£eª={˜?¯€`5ëar?æy•ixŠ?³=¢Òò8"?—œn.\?'­šW³?ѓæðB%?²Q¬Uj?èãExôÍ?´¡êã¤Ó?r4‰ª?p›]LHì?ÏVΡkӖ?´X^x^ËAGN4FGL J1934.2+6002¿çøÐòSøƒ@25Ôèû½À:ç|ò™åðÀ<«Þ7X\@ uҕ¹/?ýo"èbT‰?Á¾BuE|?ÍD<ÅÙ«@Ã$­^r?ù(ǬÒ['¿ï}'›x—?ïÿ˜k¥k?§ÿÚýMY`¿Þ)¡"I¦<¿å?4(%¸÷¿á9âyÝ;°AGNbcu3FGL J1934.2+6002GALEXASC J193419.64+600139.5?ï¢Ü0öu›?®á½ó¯?u²…ý@¥?p‡ +×¼Å?xßas¾5×?rǏ‹Æ«?ëe]Õs9‰?½a}&$	¨?´ù#K7ç?·Çn\1·¼?¯·Ü‰Z«?¦†UÃK±¿?íãÇY_0¬? VuÚé?¡^°ëhðå?™Ò©[Ɗ? dÙ|ì6`?'§2¶
I?é°~'N™
?™Àæ
œ?¶[Œsºcž?•¬48ð‡?¼ ~÷=?'}PÂøþþ?ï:k;7cš?‹HlD:±?‹9š{Lï ?ƒX<Տé>?†+–ºIÅú?|ÒN‡p£á?姾Õ=‡?ɾï¬B?Èiågßs?ÆUÃßpñã?À÷FAWä?·j¡˜óTÂ?ì"öõjOÕ?§a♈?­ðÍïøÑ?¤*ñMéœ?¨Ï·ªc²?"ø<ÂG˜?âÿiX^;?­‡~¥Q§ ?ÅÆêytÏÏ?¬ÈÝlÑ2?Î<³á)·E?¦üRc_AGN4FGL J1934.3-2419¿èÏmͧ¬ñÀ3Ìu_þmYÀ:¸£a™xÀ<psT‹r@!	L;P?ùiU~·–?Ë!Õþ#ÜÔ?Ò7A_ƺ@к%*\@U'•ñ‡¿ïÛ>ê÷Z??ïù> #Ìc?ãÇ¡A(¿¿ØáŸÂ¨†œ¿ãǂÀºí¿Ù‹n]«¬ÂAGNbcuNVSS J193412-241922?ïÊZ!¹7?j4dƒ³¹`?I/9oêPÐ?:ôº¼/?w­<áœ?hŽ#,x¯?ï äÝBnm?ƒÞ¬f,‡?aߘC:·Á?f9d{³2?ƒNâ¢]HÂ?€'É=B£
?ïNÀ².³>?ƒ±ßõÂ9?k¶+Ì:Ä`?p²ñ¨#/?'±$Eq³¨?€Â€œV<?ío»y¾1ÿ?Ž¢-Mh?'ç£c¯_?fÙ@·÷|?²%/ǨQ—?Œ™
IýFŠ?ï‰QuÇ
?|U¿®
ÿµ?aPwmõþ×?X¬§,C?‰W"¾n¤É?yÃi$Er?îøÚg?œGÝ¥'?@?y¼à§'Y?‹ÈKÜíïA?š,'žíZ?–÷	ý¨ä?î˜NÐóx?'QBÚôl?w"ë²2Y?vžon±9M?£Šu~ 0;?÷›‡¤\h?êÞ<ʜ×ù?¢º¢zT4)?‹
<G'¶?|½Ak9œÊ?ÂÖ9ɪ6?¢ŒZ'§úßAGN4FGL J1934.3+6541¿ïÿœF-r@4RmzVÞ3À9ËÆ<ÓGÀ<J<Q†Û@ߝâ)@/¸¿Þ¨?¸öç?Â,ñ$ÅÝ@¬ž#lÓ@[µ³U­¿Å\ÿµW¿èOÉkï<¿é³^™‹¿î‹1¬Jv¿ïò<'Î{#¿È³çcQAGNfsrqTXS 1933+655?ïóD4¯¬x?c»•Kù?B0—0Ö?Pozöd?P_NáZÒ?\	Åb2—²?ïފã?x7ƒt4T?D³þÑ×û‹?UцÈ?)?lHãoå¹Ø?uZÁHˆz¥?î'àrψò?ž_[ÂÉi?jC#\xÁP?vE¢™z½?¦-ƝéÅ?«""ĈK?ïûQÔwÕ¾?)oah:k?!Gzÿüûc?f°³Q¦$?<͝6¥<?&}êúOàë?ïÕ:
#*¹?£éQÏÁÎá?[Š†2n?r´Çýð?m­ÝBð¦?£ÅŒ=Î]?ï­¦·§æ?"Ž÷¹'Yû?Wå+®{žG?k'Ëdcø
?™· $?«A®ii	?íX|r	Ì?¨iÃd¯‡6?teî®ãD–?}p³u#ŸÃ?³õÁ"š?¨"Jçd:®?ïï¤X—ú;?NtQER±d?@²¾/-p£?3&h"õ\?X]ðËé¨?Iuæ\ÚÅAGN4FGL J1934.5+6139?ånãM Ot@2Í=B€®À;hIóiÈÀ<¾ÀÕGő@S>€ï(Â@è"»ìª¹?Ñ*—ëè?Ívñä^cã?ü4#óûÿ@æüõ‰"¿ïý–Þÿ)k?ïÿËô_¹¿Ú#½l²†¿è}}`ݐ¿Ú)À£s¸	¿ïÿG=¬2ùAGNfsrqGB6 J1934+6138?ï¹ù;üÁ˜?sRéc0Ô?_9¸¹<¥?R™Tå1Šù?{4óÓPp?pqË'½Õ?ï»>y–?}Á%šü­?U§˜É©?Z.Í·Ìn?}2M%ë֌?yÎ7²»â?ïÁٝ?Œ-ô$''?rYå½G=h?qrßà>³^?˜KrhT?‰¾B®@é¬?ïƒnŎÁ?já!—øu?i4Nqî&?Q @'÷³?ˆ×:þn)?iړ›?ïj'ƒÆ?'©þØîÝ.?oXÐ@x?c£=Øll?¤ÔÂ+âq?€©d³uó(?ï=jX°½š?•ÂàÙ¬Ö¤?jiúÿìÞ?vwÿ°J?•u'/'?'+uëÖ?î\ê½9e?"Ý•"˧?…Zm\€?ƒ³.HnU?¤ì‡õy¶?'Žµ¯"›?î¤UÿÞ>‡?‰šKˆNš?zÜ BíÈÀ?mÅÈë!'?¢_ü~z?‰emê•UAGN4FGL J1936.9-4720?ècTvsáÀ;ޜ)¦À9¦óp.À<
—þ@ ¯K¿F&€?ûé{DD?±¿jŽ",ó?¡¥ÓÂ=v?ò¦ç•¥ï@œO3™àf?ï{ˆA'¿¾Öh¬çª¿áJÕù¿Ô~Àdß}©¿ÝÊhÙÞ-G¿ÑÛR6-¹wAGNbll3FGL J1936.9-4719PMN J1936-4719?ï÷JgŠÜE?@~lFl!o?Ǧ–í%?
ߣ°^¾ï?O=}ÇsÅ3??)ûâ¥ã?ï猗0;e?iß3§+cj?2¸¬À,?@F:=L{?fVçß?gG_–7Â>?ï·s'¿ã?h`ø.J¤=?R;=ò§Y?;ÚÅÃÖÒ:?±vù:LÛ?g6d"ŽÕ+?ï±×S
™?^Õ3î'ö³?I%
9|3?,¬ñm?òá£Hš?^
ÛXSo¾?ïñë—_¤ù?I‹*å·¢j?/2p L²æ?ÏÜ
¾T?XBƒ¡›Å?G'=@6]ˆ?ï»Éٗ$c?'ê.Z?A	ýmîW?QóyÀ#†Ä?ùӟ³'Î?{ɬá9á?ï[®7Ç?w×vàŽK?Y*xs·?U>±Bº+?ˆÛ£ÑÂ/.?u´ãþïk?ïA"Ö¢ê?x5"T	­Ù?]õ!VBÃ?Gom¤ßÐ
?•î31­7‹?w«dÆë;AGN4FGL J1937.0+8354¿ïñR\]î@9ÄdE#öÀ:úôàM/À<Ì+
|À@ð?S	?ÿ"Ñ‹xn§?Ċî[ôt?Á·ƒåRT·?õA›«Â'@œ¶×Âõ?ï§W\Þ'h¿àÓC>C1®¿Ò8¢]ã`¿ÞpGüó¿ägûnj,¿çã¡àø0AGNbcu3FGL J1935.5+83556C B194425+834912?ïÂéF€?p´r|ג?`2
ZdÝ?U¾`÷ßC¡?vrUûd°É?kßTÊJX?ïu:lb~Ð?…žÑ=ª‡?jm‡('?iV/QW.?Œ*‰Še›§?'^©¸.‡ã?ï=^ý?Š?ñ…1æ?a/Ê#Ic%?\Þ»}s6?–9ºý:ª€?Š;S¾)?îÖÞ5>?yƒï/ à?ƒ÷þPÀÉG?_ñûmµ}?›AÅu?xkF4ÆB?ïƒGú"YÛ?‰b¢
e×?teqJ¥R¦?nõ‡ÊšÞŠ?"ûHŝÑ?…M˜æˎz?î¡¡g9õ?št÷Òç?{ÄIª¿Å?€@Ð#÷/'?¢m`Wbû=?–ëŒ L`2?î›ZZÙ.I?—b‡¸?kk­Óƒdj?e{¿s²Ò?¤"Ÿyjj¦?–È%€êŒ€?ì"ÉÆ]?•‰öµê¸9?šz?U8=J?~M'
SH?´»!ùîѬ?"ö›
.˜tAGN4FGL J1937.2-3958?á6M}r'»À9]&ú?̟À99­feÀ;ÿ<ñøÖ@@8xž!h°@è÷QÕ?±‹è.ú?²n¶l
Da?úÔní¥,@ͲûÀU¿Æ‹&ú•²Ú¿ä_ÿD]Å¿èØ^›–ÉÜ¿æö)	€¿îH' XÐ|¿ïµ*Ÿû AGNfsrq3FGL J1937.0-3956PKS 1933-400?ïñA€uRµ?RáhƒØ­M?4r6Ìð\?*ƒ´Þˆ¹m?X`qëŽÞ?P©°ž´Å?ïÛ9u}Á³?uozŽ÷â?G*Ó;1c?YúË¢P-‡?nûÕæ1eé?pÐJCdÀ‰?ï·2²Àî.?v¢ïá&Y‡?ZÀ˜{YÕ?Nš&m$¦ƒ?}¶€r:¶Þ?u嵌Œ?ïю£¤èá?Uƒú®Vôê?`F§W'ü?F@µ¤ðÞÀ?niád?N^ÝS€L@?ïÙY¦B' ?š"Ÿt÷d?Le¾1C˜³?frû\Ɨ6?oŒê0ÉÄ?ˆ\Òpº?ï‹:ßä?•d鎤s?bcO£0è?€»Ã¶0Ò¨?ˆ¢]g®Û? 9å·¦á?ÕMÐ?ùωl0?f*ð‰_x­?i¥¬QI6?ŠL<ª¼gá?€Jímºñ>?ïƒÔ»y"?vÄÏ€‰?wښ ÁµN?h~s$D?æ?ƒŽ6þt?l—k‡†žJAGN4FGL J1937.2-4217?¸–p±
QýÀ9óôým~‰À:ŒÆˆåí/À<pŠ:N@Mš{õá?ÿ ö4¥#;?Æ'7RQ±?ֱñðþ@
U°†E(ÿ?ø6+|s?ïsþÕ]•¿àñ
™¶õË¿ØŸ"ðoê¿æ¿ÞNÕP¿ëV&x¡Q¿ðAGNbcu3FGL J1936.6-4215PKS 1934-423?ç'hï?¼Þž=d±Ó?³å'oZ‹$?ªe7¬Þ}¡?Éq–x§?¶÷Ì¿[¬?ꟾëbº?¾(¾)	ÓW?·Ai¥Ë{?´C/Rô†µ?³ÆPbÂ7¶?®ÁØq°A?æ½\[ÂëÅ?°þ´æ[?ÀL>{?¦›2P(D>?ľPŒy9l?©Ibh¯—?çZ÷'Çͽ?™ðÈ!
ä?»¶Q5QÆq?'åäàd»3?ĸúÆ7åÓ?"=&‰Ô?ãMZQbѺ?À="©"=?»Êl0ý¥?°l\æ?Òr°P<d?½~ŒYâkè?äÆrªf`?Ç펚F?ÈaªÈsªO?Ĺ·Ç,#õ?ĄŠv¼0?¸zfuð?ã×7–6?µß‹óí×?ÆÕ]PN]A?­þU¹À¸?ÉÌ¥Õ½d?¯ŸíG͑?à!Ó2}¼Õ?©u<*P†?ƹ>$¨×?£<oxËÓ?Ô¬üûò1ê?¥|h]½øAGN4FGL J1939.5-1525?âv#‡05À1säXÍÀ:l`´u½òÀ<ŠJq=Z@¹UÐ-@ò…fîW?ȳ¤‡´??ÈÛؘÝÜê?þ06(°ù2@/~UñN6?ïá8ÿûÎB¿Ã
3µŒ¿ã% ¶Xí¿ê(ƒ¬ÈJ‡¿Þ.û–
óß¿ïÿÿ" 5•AGNfsrqPKS 1936-15?ï発%Ö(?[Ž¯,´Û?<E_a°Þv?0
ò*qŠw?dݙù8Ú?Y8X‹XJ†?ïßb"V¤?nµÎÌ?=K¦¡¢ô?Gî,¨Iå?lôhƒµIS?lÖÜQñU•?ïHÞð?ˆÏàwá?lö¹p©ªA?rÑþØ¦æ?"^ÅûOÖ¨?…Ì:í
u?ï­ÇcY²?`ºŽZn?L^¤f=C?2ªáS÷Èc?'È>LˆÆ?^´¾Cã%Ê?ïÖÖµü??hÉ2RQuW?Iš4ø?@:jѳ#?qaTؙ9š?f£à/?":^?Œ"5~'}?SC،f‡Ì?gƒ¤L"]?"¨ N1¹?‰#y©OŸD?îŽENNþ§?—4'»?|©ŸkØ¥¥?y׎S‹´|?£†w.ô[?•¨9õŽÛ?ïAu¸‹D?€¡PÛ«0?c«:љ,?RܺoÙÖ?biñO&ó?€ ô*U‡PAGN4FGL J1939.8-4928¿ïu‹%@âÀ;äÿëJwÀ:…¯	ëÀ<ƒ€Íù¦@þ£NÏ@~â¡Jh?À(ÁÕ¢ß>?¤3Ê7-?怮¡=§Ö@¬¶`?ïØ5jÀ¿å+îÑ"2¿ç$aß(ì¿ÐÕbÈw(¿äÆ>QÊM¿â™ДØjAGNbcu3FGL J1939.6-4925SUMSS J193946-492539?ïÝ2H…3?'¬Bibî?>Ú];¸»?S.Š­ô•?o'9…y¨?€eŽ/ô0‰?ïÎ@9"ƒ?q=ZÏênŠ?C'¬7O{?KÅ
Ø	²Ð?vœm¦M'?måÉ#D/´?ïˆ(—ñV?'T ßî?UQZ¸u¹?<ÜÐ;Ì?‹SOæзœ?þ?áÄb?ïžgœqeH?_°d$Úb\?Y²"HN1?9ËY(]õ?…/ÆsÀD?^k˜×^?‹?ïÊÊqü¶?qÊÇ9g?HˆUB2o¶?CÑO¥í?w‰í‹}†ò?n¨
Òó!?ïgѦXøG?'Ìø6u?Q»rIÚý°?a̜›ï™²?'êOº@?7wc½…?ï+YÙÿÔü?‹(¼ROZ?awÛe~x?R¾—`'?˜eàߝAÁ?ŠÂ^³	oO?îÚÔ[{?«?€)XD3ék?tþv"íî?^'A¾^È?Ÿ£ôøv/?~øºú"ñbAGN4FGL J1941.3-6210?­›H4;	ÛÀ=‹*{ԌµÀ8	j#ŠHÄÀ;½G²Jk@ÚN#yÌ@͝€Ú†?—ËÄLJ±?±­­ê‰@»Šãq*@hŸô|"%¿Ä|1>fm¿â΍âVKç¿æK<>t°¿å{f¾%7¿è-••¿ì®Ö­ _AGNbll3FGL J1941.2-6210PKS 1936-623?ïÎD˜Ø ã?¬µw'%	Ž?Ví•'RÊ?Œ²Fjœ?s"nË×Ý·?¥¯S`Âf?ïä#aj9k?kIøÇ$‹?6ÄD?G€
}—m=?iˆ|?hø^V
±ü?ﵪÌ`Ò?{À"k"Á?VÂâRB™?QOÖ­ýMü?yáI±ÑÖ?{
Î+:ü?ïü…C˜¨z?"Åm)ûˆ?žÎª¬Š?X^çŒOµ?6î1
µ ? —ìæw!?ïÅÝ$¼U?sbwCôn?J*t)÷æ?@¶l?µN?y̵gð?r1fÐ$¸J?ïº+éy?'Û©ô¯Ž©?OU2<¸J
?e𱯠¨?~ÿdß[¥W?€oÃ1ŁH?íN'L?'¾@¢œtƒ?Yã•Çk$?Y[Q°>|?"õ¨6‹‰?'=õ@¢Ê'?ï÷þҌ?@‡¡–'Ü?(eŠ«‡~? Üá7Ahü?Iën~~$‡?=)ƒân8ßAGN4FGL J1941.7+7218¿êwìwPÞ.@6©£Ò؀À:J¤ˆàä²À<¢—o@Í Øè@|lb(ê?È°`¢|?É2ØÅS†»?þ0¨ú_­@Ÿè)Ê~¿?î¼#Òm¾¿çk6#¨|¿èÏa!Xi¿ìn	"&¸Ñ¿ÔÅ
á…k¿ïÿ]þ¸Ø#AGNbcu3FGL J1941.8+7218GB6 J1941+7221?ïãA&wV?j'PbTœ,?MãØù{íA?R˜.Ö¬?eEã]ã®?c	VÁÞ×C?ïÊΪiíÒ?€³ùFqa>?UòlO¦´Ê?f».Xœ¾?uÓü!¿?xŸ&£¼2û?îõ{¢ú8?ÍéÏ´U)?ƒy¡7Xý?†F¤²¯ó¬?—"¿;Éí?‰õàO2?ïÜN¾m?P콅jŽB?:0g®­ÈÙ?$τíI¬?p5ìÀ™øä?P\ŒéÌþœ?ïÍyb	z?t^ÇðžÕð?VzXá@•Ó?X\•ÁkšV?s¤¸Ü'ý+?pÈcxv¼{?ïjœõڒ?"«"K"–[?i­º_Ð0Ã?zÜ®{ý—?ŽíSöMl?Ž›¨œÔ¨?í'ìÜBø?ŸúNÂ:à?˜ èb<{ª?"Yè9ö×ô?ªÀ¾‰y«?˜°ŠÆdu?ïy6¢©bº?w{ï›øÿ9?XåwÕÚ֐?L?­v<­?Ž•¨i\ƒ?v¤yF:ëoAGN4FGL J1942.1+4011?Îhüe85s@ ¯'Àa"À:¥]òú^À<^úaZŽ@µÈNbä@õ‹$‹Ðƒ?Á7ÉðÏ`?¼2^½¶Á?úƦå²@IÊS˯?îOd1¿Ôʍ'_d¿ã?Èl뻥¿Þ°¾ä¬½c¿îÈi[
lÐ?ØÕÔ]dßÿAGNbcu87GB 194033.4+400351?ïqU2À?™'ÖÃøf?\©|vÚ8?WÛÎû½C?›0Õ;Úl`?˜ˆºÐÖ.¼?î•áK½vK?¦ññým—?_³dL=@?lZ^ºr?¥¤Rkmó_?¥ò¬¼S[[?î"Oï<Êr?•ùä7@–Æ?‰Kð»¶ÇI?ˆ]:Ï9? hÝE§?lk°tžÛ?ïyð£åV?gÎrl±†?h3À†IY?J- ýð¦˜?‹w.•e?dÄù«Ì?îe– #$?¢ÃB+ëã‹?j{(0Ö/?dohYañd?§þëx¡‹Ý?¢^¼"_?ìQ¤Ù¤Ý¬?»µŸ¯?m…ËÁìí?'€'.Á×w?¼Š5'»?º;<8?í­³²I"È?ž ê
";?'×9"¦ ?"ïeÓïV?¬9(¢óm?˜ó!–æ|?îwëîiïL?"wN­mz?[ÙùeÇ?i)(¨Í·?¤*Jž2ÿ?ùÒ0
_ÌAGN4FGL J1942.5-5827?ì-"J
nÀ=rˆXÿu—À:ÆGœvìÀ<'§4ŒÏ‡@ü HtãØ@D¯ñ¥Ê?ÈA¡µòÁ?¨ÆÍYd >?áz`ƒÎV:@¨L!Á›Á¿áë¶!d©£¿è¹> #Ìc¿àŧ߭z!¿×šFÓ#(#¿è?`Ónu¿ïÿÉ¿&FAGNbcuSUMSS J194224-582824?NGá–?¿¼P "í?Dé­›â?:² ¢fju?¦#ÆÖ)"?¿¿â¡¨åE?ïÐ9èb?r|Új¢¿?AkìUH?I'êu'S?uµŽKÇ?p‹¬y£¸Š?ïpâ·Æ?~‹õͽ.¿?`úQ—?\œtgO?ùÈÙM8Ã?|í¨ïé?ï®W)îý?^L¸ü›N?V‹ÞÇ«bµ?6•n6L?˜¹®ç¦n?\Äыbq'?ï%s•o?°féôùÉ?]BÏÔ>à?V}Ý£d)?™}|⼓¾?°`Óå˜I?ï]b¼¶?¿flL'°?T´Á´/
?`W\eS/?"qŒ¶çp?jm=±¼?ï`CÀ&Õ?‡…‰ÚC^Î?k°[Òä"?hš€¾é?›1¡ƒ`Î?†WŸ>Ã5ÿ?ï3Kjr˶?xÚÀ8^?i5P¥Ò–?TAF¶»šù?–o袱P?w†vB!Æ£AGN4FGL J1942.7+1033¿ÛÀN~'Àsºc=¼úÀ8'%³ïáÀ;\Ì.A\@ K媔=º?ýWo£&
V?¡D{@N_ñ?ž@}@¢?ý™œô˜@֛Ž¼Eì?à@%‰ýDd¿ÓošÂŽ…i¿ß¢Š# ï¿Øae?õ¹U¿Þߟ!î½8¿×Õó¼ûžqAGNbll3FGL J1942.7+103387GB 194024.3+102612?q¿ú›?©@\Ãš?>-žÔâ½?2MD`y›i?á'*M|?~üA·ÿb?î>Æw{À?«¬FÖaœ?MP€¤°0s?^ÄÞ>€Ã†?«¨Á™µ'?«^m¬H ?îÝüEhó?"V´d¤?d¯Š/"#?kwÚQ¤ž?? ä7˜4Ï?"£ûiâ?îҋ뱉?€'0z¨ß?m‰³²<
?OÍWy L? þ¦¥t0?~†~ÄâÒ?î­zì:—?•ÞÔ¬ØB?R	ވ†€É?HWß6hg?¤˜G†f?•h:Îs?ꙉªýÞ×?ÁÄí
ëý{?[FQ/¶é™?p)
é˜M?ÅcL±ðŽ¯?Á¢ÚP#À?íð³=Hy°?ž»‹r>ªÃ?nók]Î<»?t—!9?¯•x8®?žN¡OzÏp?íd0íl½?˜L¿=›€Ÿ?€¦§ÈQ*$?h !=†N?²É£ŸóI?–ý´KL0AGN4FGL J1942.8-3512¿Â"/&–îÀ9!zg¥*ÇÀ:˜£ÇðÄúÀ<7β€m@ôÃ@Z±'Ýãv?Æ-Èe4L?£"k­"8?ÞÜþ3!@@
2žb×?çQj‹¿ß]Ò®Že¿æjußÖó¿Þe¥
æãϿ֘…·d†¿ìƒ<àÛødAGNbll3FGL J1943.2-35101RXS J194306.8-351001?ï›HÇÞÀ.?~%½¹ê^?F×¥œâ)?6‹¬'`èh?‡ÀS½xcB?}uêiH¤?ïŊëس?qØå—!"?FHy²â?Jä†Ûk"®?zq{;4\r?p*Ghª§t?ïrO
Œä?z™:8Š?]Āà֓!?LA†aä¨ý?³¬‡‹cÇ?y ÞïÿtÇ?ïgªªËµ?fºas	"n?PMšLW³V?2xàä?'ãÆmÊú?fk nF±?ï¨ÞR9?nöM'½´?X"ò_á@'?K¼"+ѓï?œ¾Ã‹	Ó?ŽŒœóû–¸?ïlX¾æÇ?Šó#n\8—?RBbeó?\¨"§oÊ+?'PÁù\?‰á%©š´?î•wml6?'J$ÄãýÉ?m¹/—y?aûì_»,¶?¤Ìö.Ä.[?'¢g¨fÙ?î0—l"­?"1@ˆn?fœ:l&0?Tÿç¤?«ŒËXm$R?ƒÖÿôÃLAGN4FGL J1944.0+2117?֎{׊s¿õ
WqÖÝÀ9Ÿ©,£ÍÀ;¦I†[Ï@#Lo'*;h?ô…UÅ.rÚ?Á`Ü8Ё?Î雥"c@Û£)eT@~¿[5z¿ëgÑÀ§zƒ¿ïé†@÷A?ì~ò¹Æ_Ë?ïýßÿ¯x(¿ÆØB¡»&¿ÎÅͪAGNbcuMG2 J194359+2118?ç#ñ
ç+?Æ9ŽS€R?–à†(jÜ?¨ýkî> G?ÐJ±|ö\?Å]&ـì?àÅÂ'k2?Ô¸^ø^²?wíö%&NJ?˜DÖ''Ì?ÞÃéEË´?Ԗôx¸M?åðSØ\?²:#Æ¢Ÿ?›kJ¹¨?'ÚË-´oé?Òm–˜ª¨­?²1¬]f–?ë*†ü*Ó?°O7&Cð?g‹Žì 3?a³Â£÷Á?Â÷·Å\H´?°M"ÀŠr?Þw² *ò?ÊߣôuÄ?¨ÿ/<ÜéË?°ÑFRK†¤?ÞhgŠJ•?Ë¡h£‹¡?Úü=rý"«?ÑÓs8˒T?€œ"î?¨±"0¡•?â
ƒDSÓ"?ÑŌ:¥1A?áùP/\'ã?³È
"÷.~?¯/§n‹§R?¡Ki2d$n?Ø'j³ä.Ï?´µ¢Ô?æ.üá×9Ò?ݛ ?†<gCÃêŸ?'î½_ü?Òð#üsG?ÂqPàÑMIXED4FGL J1944.2+3921¿Òâg–ð¥x@V#ˆÀ:5ƒO«8þÀ<+øàQ@>c†ã£?þG.¬?ÀyF¨Zý}?͐ÉE.@ßkã}é:@%ˆà%?ï¨ÙÞ-Ga¿Ô¿·%Á¢¿Û7'"Yœ)¿Ù ºKâ¿ç0²ð'´{¿è֔aKtsAGNbcu3FGL J1944.1+391987GB 194223.9+391242?íwFEÏ¡? Ž˜a?—p±*"%?‹¡y…ÿ"1?¬ÓEù
¼d?™üR3o\?å1HYàñó?Ä>ê­¥?£ÝÀåãÊ?¡OrԿҗ?Ó9s"!_¡?¡!o³¹x?í¬"Ñ?—¾ÚêÉlX?"i"HùDÚ?‰óD¨x?«
öO$?"…ÿ_¦l?ëÇVžÐÄ?‹ª><·0?£ÁÏP‡BY?y°E½¯d?½0Ý¡
¸?‡¢´ëò'^?èÐc9mñ?·¶¹—QE?²!ÏI$?¥ôԚú×G?í‹û­)?±Û€ 4¤‰?Ú¹·ÏÃ*?ÈUÜ&BE0?°'="?°B"%ƒ ž?àìÂܑ™y?ǒ‡èÆå?éå[WO?«>{äØ?«eœ¼ä¢W?œb¯S"q?Á'+tUšð?¥HE½D0Á?ä±±Ùg¡?  æo);_?µÉ´CD÷w?"wzi̤?Ñ+e‹—oÀ?{­g°' MIXED4FGL J1944.4-4523¿Äî'VSk.À;ãü–þµÀ:òŸÅ,ÅÀ<aV"@!±ð°.\?øœ5Ċß?ÃoKè5Þß?À¤AhU(ü@³;–¯Ž@K-Kè‹Å?ê9!°:?ïÎ~T–Z¿ß€ aIq
¿È"CÄOû–¿Éö$_ó/¿ÓóBWhrAGNbcu3FGL J1944.1-4523SUMSS J194422-452333?ïTB£yÓg?¦ð^sêÃ?L/RþE?E[hÎL?"–0øS4ò?¦ç¬ÐlºJ?ïÉ4F%Â?wúP\ô€¦?G%Hòá¬&?P#•fp*Â?x3è"?u¡~½ç«ò?îã…áUðÍ?"«á¦ÀÌù?Xbˆì9Wò?Fëæµzǧ?¡¦˜Ææ?"ªÛ
•‰?îÒ§Þ'ý?~¬™Ÿ\q?jÍOØöã?TôHu'd?¡(­%!ö?}åûx+Ö?ï~~hÄB?•M·éœÙn?føF©®ÎÙ?aÏ|@Ü?™q'ftžÐ?"Q-%Da?ïlüíËö?Q	ÑȲ?XM'0Ȩ?b§áäÁ ?Û—ÜNKÈ?Ž(Ý@xÆ.?í»2G>Ç«?žB'Ϊ\/?bàf{¤?]~Vóé	?±j"
Œ?žzט ?ìú§ôc{?˜/ó¸P@?çr(àµ?qØj½ª…?¶,OýøÏ?—›1jY†AGN4FGL J1944.9-2143?îÀéx:_‰À5ȊGìÿÀ9:._ŽÛÐÀ;݉à¾ò@ di¾µ‡â?üYÝÁç–?®JícÙª?«>Ÿ'ª?ÿÛÇ4Ý@y؜ŽÁy?ïíj Ûç¿Ñ*Ÿµg€¿Ùêã"ύǿԠº $x/¿á`‰þ#r¿Òr¬ÅÆHNAGNbcu1RXS J194455.3-214318?ïù†Ov ?=-êtT?&™ß9Äî?¥M"ÎÒ¸?GïÜMß?;ç¬Àö|_?ïëÔÿ˜ži?fYŠB^(e?.,)^9û8?<%&™ ?bH=׊·?d\Œh›¯O?ïŸe'™ns?yšÑ§ýàk?\%áÅé?aª²oK5â?"¡ùﭒï?wåaª¨'V?ï¸Ìô¥ë?[³nœµÁº?FŒïRÔ>Ç?(ôÆ!ÃZ'?€d-'ª?Zâ4÷YA~?ï÷=UÃMj?EüÕ÷%
?!#€xá?­:B?NÁé(Öîy?Dt"GÚË\?ïœm÷ø?€|ÁåÇ©O?E÷¸z«?XO|[°?{ó¥O¸?~Ð}Ó·Äõ?ïp¡ª×{õ?ƒG,[ÊùZ?`dÃ]<8?``Ý׉XÍ?¾doºNÐ?'¿ñi.®?ïZ7[-p?w;8•E{?YsêˆÌy4?D®ðCK–?"%zmAgx?vyi2Q–‹AGN4FGL J1945.1-4007?ÒpöŸ{}FÀ:Þ*<êlÀ; κÖ¨À<¾€íÑ)S@éé%Lk?ÿ^½çX?ÑÑT›ã Ï?àùJn¹?@ê¢þ)q@
u?Öڗ¼¿ïÿÐ?sŠ?ïýáAÎ×i¿À¸™¹úã¿â–Æ ¸Ç²¿ïÿo·HJ?ïçh5'‰AGNbcuAT20G J194519-400557?ï¦,¾5@?'@ĶXQ?€ ²¤˜ÖD?Ž ôâx?iPw5œg%?h÷uä{ô§?ÆCú3?…ŽÚº%t<?bŸA›û!‹?oY?ézYš?ƒk~{hÌ?šÅC6¥Ÿ?ìb9i
ä?¦â?¦Ž=©?«§Æzoª)? S:î/?®4¢ó*Fµ?^ñBì?﨏þæ$?gïë¤ð
"?gÔÈZ&†	?PËÁŠP‡Ì?͜PB¾?cjÒmµäù?ïr¢œ*?.á¦ùà?Š+nÚ‰U?Œ}œÏ3Mm?rWÔ[™$E?pí)—0¼>?îïü¾…?£È%=Cß?yèE¨xÖ?Š¾Ï"c?›†zï9¨%?¬É–Y?ëævÓ,I?ªc©u>Lj?±ïÛé4y?¡Ž˜a?µ8ðbXX¿?£• ??ï4ôX?…@—6ø@—?y½2ZX+´?hÍ]ÖãÙ?˜-ŒÃ+ë?'¾ZŸWüpAGN4FGL J1945.5-0153?ï*[¾ö(À)È
°ö­À;!C|V'´À<9.¿0@>ßôñ"@ݼfM;ó?Õÿ\÷§Â?âQýŽ5¸I@mczù›b@ÔQpµõ›¿íسà¢ý?ïÿÔqܼ¿¿‰c˒¿êDm'ºZ¿ïýibDBпàÇA<á1ßAGNbcuPMN J1945-0153?îÂrYzH?˜—/³¬'V?"<fô¼ç
?ŽíµêKýs?"uMëãkß?=Žqk~Þ?ìaæ:˜=Š?»(¢dÞâ?¯oKˆÏe?µ"f €»?ªrPÎ{Wø?ªR
ü³hy?ê"pcÈÛ?ªaÑi/<°?³æÄ¡ƒh˜? ÷üÐp|\?·€ÇÚv?¡i@*Oz`?ëR?¡ðD?™/ƨV±ú?´gaZ`Š?'¬=šœ!?±¡–f~ý?'9 c!n?írãªèT?¬SíÆy?¬?æä¨?§¸žKó´?£v'¤?™cJKTq"?睰[–Ãj?Æ.9cÎÜr?Ívm4¦?³ÆKSeƒ?»÷o{c?ºÞݹŒ±²?æ^:›1tA?´–9¼?Á¦YN.?ª"Xd§Ô?Åk…ìààÍ?°îPÛ-Æ?åŸÄÂxq<?¬‹Ùwâ?Ρc<T?¨ß¶êzl4?ÅòK'᪼?¨¿búÒyAGN4FGL J1946.0-3112¿ìõbÅÇõÍÀ8'ÿ.Hè§À9wQŸ/ÐÀ<	ûï»@r*$Þä@•a[dª¥?²&rÛiȜ?ƒNcnÝÙ?ѧé=›Áè@#â~å¹-?À~Õ]•¿éýaw¿ámÔº.¿Ùˆdà
—¿é:aûš°¿à;š{pdAGNbll3FGL J1945.9-3115PKS 1942-313?ï€ä¡!DÁ?€Ë>Ä?AU?d¨óÛ*ÇÎ?ZEȑ÷µ>?Šœš³}£ø?~5 rå?ïʈEÎI?{L·^?N@ÖD"œ?Z¾Td›â?vóÜ+¨%?vêgîÍçÎ?ï+:–ÝZA?ˆÆÄ2ó?q'§Ô»È?r£¡qÿ¢?–4C2탠?…=­¾cl?ïUça½N?qž%l?l#üâd/?P;a÷²?'¾"Hùxd?mñúûÃ?îj¥Æ×? &¼z–µi?qçâ'?wHœ)Ö?¥Áλ?œìTì/Wu?ï^û/Oh?•§¤{M[?_Qáå.ä?sÍD`ëôÎ?'/'\{±?'ïôb¸o?íîYcëÚ&?›³êÅ߇_?"š^
ƒY?ƒ8"KÓiÔ?«ú',Ô?˜õõ…À®7?î_!ÚV‰`?‹ ³‡_
	?'š!¾fŽ?m:B÷¿?¥gYêýÆ\?‡\
½šå%AGN4FGL J1946.0+0937¿èh£Ì'./Àõ@‰]À:Ucé´d À<DF€íÑ@ D§•ßc@ÚõýG¾Û?Áò¦%C0?ˆäŒ1&=¬?ȪJè\@O7 «1¿îAÎj[¾?êÞæu¿ãŸD(y¿Ù]$~£²¿ã·/+H¿â(TÐAGNbcu87GB 194328.9+092856?ìZ°°a‡/?­í¦>¬"?t›³‰¶ Ü?b&à?»à¿C³o??­¹Ðéë?ë@¸
Ç?¹€ŠêTG*?aü7*Zä?i:°q¡©Æ?Ã{CbÞÐ?¹?+Y"?íB÷R
d?žxzl#ÿ?€S	g]?q¶Ë5Js?³ååó³m5?[Ø´ìÄ?í®öv®!?"–P™2‡
?•ŠŒ§•ö?`>i¹Tdy?°XÆüLm÷?ƒz!Šâž?é6[(<,?´Ù"¦¶?‡ÂÎ)ǎ?v—u'|î?ÊCæ³l˜?´Š`À¯ê?㮄ÚßE?ÈC+8gûg?i…Ów4Œž?{††aœë?Øoì3f×?È6»à¸´^?è¯ã)|óh?­àbD²{W?·ªîÙü†?€QòÓR.?Ë)}ý±Ç
?­2iÁ‡Ö?ê"h‡¨ÖM?šüiƒŸ?"¦³Í;Kt?yáïÉþó…?ÃY‡gµ=[?™Øz½-:AGN4FGL J1948.3+1207?ïùõdúMÀ.Ü ý¦‰À:ˆ­Ú™>*À;ô"ªlO´@±)bNÿ—@=sãýjú?҉Uê`o?æ
²
©§@/'…€!@BZœ¿ê?é£%¿,P@¿ã÷æV
ΐ¿àüÈþau¿êèNòÄ®¿í¦i³Ê¿ïÿâ–é¼AGNbcuNVSS J194814+120645?ÙítPù‡?Ã>‡øåâü?ƖyǟÄß?»4W(8‹ë?Û°Õ§ß$
?^ `Œ?àÖK"Šà?Åe*ëÕÀ?¯ýþ¸¡)'?¨9ÏJ#¼?ÚS©ãò5ñ?Ä#\lxµZ?ä€àž¡ýR?³®–óûN?Ç©AB?°NûˆÂŸ?Æ÷ÔD\È¥?¨|œ¬Ë.û?åÅáiÎ"?¡ªÍ
¦;?¹Ø7Ø,+?'Kf°¹é?Ëü^j™{è? næ
|?Êÿ×6ï;ž?¹LHG¶ZÂ?ËÎOùèc×?À	e"i0Æ?âLv3Ê#?Â0w×|ÿ?Ò5&vûù¥?ÅðWҋ
÷?¿Bá'ï¤?»F2"QÜ?âý'R9?ɐ™;Œj?Úâ}nüÉ%?¶åÃK(NQ?Ò/ìðaZ?·ŠâíĕÑ?Ò할¡ÜÅ?°õëé-?؝ê8H'?¬ºÆê#Ž"?Ƌ5¦úD?¦ýhaj?Üzçt:\?°'ÉNd¨PMIXED4FGL J1949.0+1314?Ý$T¶zÀt/è%çÀ9nç¼<[ÑÀ;˜Çÿ²|@`M"ÃÌ@ïÃqÚ7ï?ºþy×ÝL?¾eà¦@æ<$s|Ï@›®] ïú?ìö쀜GŸ¿ãÿ!é^ÓË¿ãtßp=½¿çIH¾H¦¿äé0&Ž¿è¥
±3êAGNbcu3FGL J1949.0+131287GB 194635.4+130713?ê•øE²¢æ?±p—+é‡?rÒóÛb?qј¶ò§?ŇJüAs?±UC³-öP?çf t'?¾ÜZ"O$?†Ñ²K?'û¶¶µ/4?Ð|1‡j·?½=~ÌÊڕ?ì7b\8¤?¥©Ùiçp?‹Ü~¿¥QF?€â‰FÃt?ºÉ]Eo9¸?¤H^Ùù1å?ë.+´0@1?‹cǧSS€?^jùîÐ?rÃ=æ6ù?¿7Âu¨E?Š'ÄúwS?ãŠ|WÅ?¿A~ê/¢õ?'b&g}$´?ŠÛÝo¾?ØÖȠ劫?¿)1ùsÛ?Þhê> ¦?Äûžê"ý?"¦€¾É'T?•CQë-€¯?à&VÛàz?ÄÆÕöÛØÈ?å3«º>»ä?³þ›X¹ê? P'µA\?Šƒ/€éLõ?ӎ–TÚf­?³?tÚÔi¨?äZ"²:a? f¢Èا?²–¹7å?΂Dîf?Ò|åPHº%?žÊ"úÏ_;MIXED4FGL J1949.4+1247?ç%³HAbKÀ©Oð\À:‹n}ŒÙÀ;¹rl.'@ŸœBk_u@gFBÐ_?Ð1Ñß0Q¬?ÂÊ7F=Q?ô‹Ëz½5€@®¡É=÷¿ïü2¶5±"?ïûçÂq¿ä¡>iÈ¿âÄî|Iýz¿å±[Ývh<¿ïþñ­VåÀAGNbcuTXS 1947+126?ï,	Z
§=?'Tl%í?M yòÓ?IË¢î?™–¹¨?À?'XV'Þ?ìÇ1®èz?»®H£îîF?WENÖ·89?hj£2ܸ‰?¹i]O k?»?äÆh°?ëÏábÂ(??¥ÿ|¼-7?±¢•dØQ?Œˆ€0€À?½ÊÀ˜‹ýz?¤4Š›*ç€?îÑ@w>zå?~)]¿ˆ¹?a¦ #/´À?F÷¾¨Ø?¡ÑŽ†Äj?}±$ql³k?î–GAT€'?œ%0sâ¼(?^ÇìÕ¶?W
¨ækÁÞ?¥¥S¹Ÿû1?›™w·{ê£?èþy˜¥ÜQ?œÑv³CA?c.˼Â?x±øIY?˹a=»*?ÅiXx£?éŽõs,?¬Dœ¬Ç¿?–¸Kl'7½?'ɬZ1<?ÈĨWßÚ?ªÎñ4«?ìðÄ.åé?˜Þ³ZϞ?t\†µÐ0?bSUÚ«q?·9‰|´¸?˜¢ØvhAGN4FGL J1949.5+7311?Áùœ…ÿ€@5ÕU>öµÔÀ:WçG¢VÀ<݂ýuâ@Ÿî)†Œ@͒tâ*,?®Ãaéÿã?¿Ú®ó׏?üØþÒ—@Nޞ†hd¿ß¿1×JÕ¿æêG1ù¿ç`N‰Ðκ¿çXjû ¿ïÿÏ=ÀTï¿â"h\૧AGNbcuCRATES J195016+731028?ïÔ5DìV?€ß`ŒØw?^Ùã‰-b?aÝ
±tNØ?l^.}~?yÞR´ïg­?ïs/)¹6î?–ÿêڟ‹[?uJäðÀ'?Œã êéë?ˆ.'Úw?"³^˜ùö?ï¡]¯Z?rê~Y'\¯?cÍ·.Þq?_õ&õŎõ?'µ2A:ÆÇ?m­H]Fï?ï­ø(ù§?t"<]~?"Þ§òvY?d.ZÂ'‡?•í]‰q?o+,É͗
?]œ›à?}+Øx?užÏ[@ò$?o¨2Tä"?íÎuª?sæ¿û¢µ?î~¶?}Õ?¡"ÔÐý3?ˆ> j<`Ž?•GMÔ÷?¢óð'Dè?™èúáÐB?ï:=Õ¬?†‰>0&^?uâ[ëg?tΙ»³`ô?"wçû^£?*ü²µuË?í3"=Jt?'žÆW§V¨? #:†¦‰?"C±ÃÏ}¢?¯iŒ¨ÈË0?ÆÆ܇@AGN4FGL J1949.5+0906¿èæ=öÔÀ!? §?uÀ9·
Ø/×^À;ýžvx,@ X醖Ý}@€©Þ‹;?¶"ÁI–¢¿wä
¨‹R?Â
]v'Ï}@
$ô)Ýôè¿Ô"mè2Ú¿æô¸Œ£è¿çÏ
Ÿ$óÕ¿ÍHuûìÊ¿Ýqœ¥g®¿ã=ȝ"#^AGNbll2FGL J1949.9+09071RXS J194934.1+090655?ïÀž¼ÕD&?në:v"?;×Ç¡?+w€íÈKï?}ó0Y|,¨?mä(¯ÞÁÍ?îE'͂	?°®®kÈ,?@0ºnŽ›"?RoAÿnR¡?«lÀ>;R{?¯ç_£"=k?ï~ÑR~¹?ŒyçøwJ?`Wï fk?Lªl"ŽbE?›¥'Üá?Œ,a¬ý«?ï‰CöyïZ?fß3¥s•m?K@¢ê-Eó?0/WV;õN?‹úø1¿¬?f—ú?œ,,?ïy_?ƒÞuwk"l?In]ì–Ø?:wt×?-:h	=?ƒOÃHï?ê15Ø)!?ïÿ°?P'7–â^?bÔ­zú?Ç»°Ö?ßáÇ°®3?î6ª¶øO2?—ü뜡!?k,a'PT?hu"—RGÆ?ªâ"i›þb?—Â8°[ä?î¥ »-àZ?ˆ	rRTw?e'Çe¨{?RèÀ߬*?¤UÒ´19M?‡g(ûnBJAGN4FGL J1950.6+3456?×ô¨ë#Ø@&!`¢ØÀ:±îX7ÏzÀ<.ʔ
hž@!P¯ýˆ¬?üâDhå?Ó«'Ëöãø?ÁP±ˆÎ›.?÷X¨ø².?ÿG˜ÛX«¾¿ïþ9áùâ?ëa±Ë¿†"?ïü¾A™¨]¿ç(Îàù)¢?˜!ìf#¿éßÓÚÞˆAGNbcu2MASS J19502776+3456224?ëí×K"_ž?²9½¶&?dB'ž¨ÂÄ?V.ÚæÅa>?¿ï4kA—z?²$µI?a?çä´Óöå?ÉQÕP»¥?tˆbC§Ù¨?|`LœìÚ?ÏÈé¢_T¾?ÉÐ|Ý?ëÞw"\‡?¤Wýx(j3?'·"àá?xó¥jdx'?¾ÌµT$b?£éHX‰Y?í`²b=aà?•©b¿†ËÞ?iWÚDu?_(ǜ¦²8?´/®ñH
?•k¢)Nò›?å;ÛSßa`?Â^ÚZBÛa?ÜD˜B"?rH€ú÷º…?Õ9ç#Ýw?ÂSž*Öu÷?â¸Ä­"T?̎"Îuæ®?‡*îläí›?–´I^ä?ÙÕ S¸+?˼ù<ŽÈþ?涽w!þ
?²Zwá15?'»Éâe$?"è¿œ"Ô?ÑvÈsÌ«j?±¼	çýƒ8?ê‹kEÉ7í?®å)í:ú?p"!5$?qžó‰ó´?ÅMºB‡Ü?®™cg#<ÕAGN4FGL J1950.8+1211?íFï‹Ã&À!úvSCtÀ:دYÀ;ȟ·ÀÌ@,Ža'&@û
z<A?Æjt!?݂Bdÿ^@ítýØÞS@°7êê¿é°ò¡G¸Ñ?í˜{V¸sy¿ä–ù¬(è¿ç(ÒÁ&¦¿ïÿMéDÓ¿ãÒ ß²CAGNbcu3FGL J1950.2+1215NVSS J195059+121316?ŒF¤‰?²XÆ5?à/€ðš A?Å*€KÌ}?ÖZÚˬÕû?Ü0åGX?̉_¶Z*Õ?Ãí¿‰uè˜?ÕA¥W›{?ÄUº.'?ÜyÀ{O?ÅÝ2mÚ?ÕµqWl^´?±Úي Wy?Õ¶iÞëÞ?²F'Nwá?Õ.Ø=¡Ô¯?°Â#¤RÊ?ހÆÌ$'Ê?¤ýÈ©bÌ?Óª.é2Å5?¥€˜Ôá?˪—wç~?š[oþšÄ?­Ã}£æÿ?œ$•³zú?âFrqÞï?Ƴ,8~\ã?׺«hŠ>C?Åûæ«E=¢?¹ÊûçA˜&?¸ZŠ ûZ?Û¯òÑÄ-l?˪ˆ+'?ÝÝN4kl‹?ËEµ¥Ø†?Ç¡¬!?©̈*ò¢?ÜçÞw*j?·•ð¼/	?׉¹_ '?µZŸ 9‰?˛-cC?¢˜~ïý±û?Ýñ¡3ß+?²èRùÇä?Ô@Ôè5o4?¬	êO¹pMIXED4FGL J1951.8-0511¿éÌøPߥÀ/–¤D‡À:Mqåöi~À<¢Ô«¾_@܁Ðz+@)2^!‡?Ç*ÖØ¿IW?ʘD/ùŠ@¼]\Òi@8lýv?ïö¶^Ì>¿®^‹{ž±Ü¿ä«¤=âc¸¿ã_Cý…Ò<¿ì]2K­¿ÏÛ¨ï³AGNfsrqPMN J1951-0509?ï|wãøs«?£5müÝ?fçŠ#>"l?z"®«tŽ?‹($tDµ? hìõك?ï΀VL­?w$ºÄìi"?N3›ñâ'Ì?[Ù2ºc?tù€ÝԒ¯?s^\/—y"?îú§qڟ?"B«ë
§?'ÍýïB:?'ä: ƒ÷?—DÏF–ì?ŽóÑH‡ƒB?ïSý¦'+?kj'6£&?fUŸ"áxE?G8Rã³?'µ—9¬ž?j•È`?ïZ¯"Mqš?‰{Dø`,?s#'Š;l»?lõzoϝ?ÂQßö¿?…*…ff#?ïo›ô	I!?™æݚ$ƒî?k!ôøâÓ?ƒŠ¬NLž$?P…ÏCfà?"/ç-´Õ?î$Í¢4ȵ?œ2aØáMÐ?ŒðF\WZ4?‡&b€­ÙO?¦wDÁ·+?™öÌHÅ ?íòÝShîè?qj¼¼}W?¹b?æ°?d7}ÛN ?¬ÚþºO©?‹Óv|aAGN4FGL J1953.0+7651¿æ0ª}þ™µ@6øäd™ÍÀ;TÍ
à-ÓÀ<±
?x@k w™¿"@pðÀÇÛÌ?ÐÙÖÀÁ{¶?̓{~% ?ø‰Z¼äø=@ã…"¿¶?Äßbцp?æ
ÇNފ¿ãxÔ'4!¿ÛŸ¯È°š¿ìô_î} ½¿­s£æ¤AGNbcu3FGL J1953.4+7653WN B1955.4+7642?ï={ln#…?Š«òop;¬?#(ÇrŠ?s'‡X <b?}ü':?ƒÏüZq'?ï2šbd?ç8cÕè?{µ`æE?wÉtôåÂ×?'æ»´—8ü?ŠAgàVDð?îÞKïAÂ?Žæ^Ó¦Ùê?€ì.©QX?yko|{?›É?wÚÅ?Šyij«.<?îocn,?€f‹Ï%r?Øü‰g˜!?j¥›æ?¡ˆ1B6?{ýN¯ñ`ß?î<ÝB³%S?Ÿ&ò\?"Ô˳mc?Œ"c>£0?¡ÇÅöË¢ ?—3^ˆ=Õ?î
#èΜA?¤'ŸŸJ¼?ŽžÊYJ·?"µþ
N»ä?§†ݟu)?œÚir©M"?í®1Ñ´=4?žaŒ`@ʅ?'x´i¹?‡}r	j?¬™&×*)ç?˜sîý2Í?ë§ÿGGÑ?˜ma?P›û?¢}ý)"?‡À#ȼYÓ?¹wÇEé/?–4ÕyÒQAGN4FGL J1953.0-7025¿Çw"×°"À>–Œi/nƒÀ:PYddIÀ<eî \+z@îl"¸Œ@vg=%û<?³ÆÊ¿¬RÚ¿©§Çà	k?õÓ	AÈ!l@õdW"¿ãc¸6<Òï¿Õ'šCÅ
¿æŸ¤¯rÊ¿Þ½Ÿ
ò¢¿ãžlґ1ì¿Ø<åcœˆAGNbcuPKS 1947-705?ï©S(¤—'?~'ƒô·?Q¯a@Z¾?HE Ec/•?ƒuI´¦#¹?|BŽ¡;Æ?ïšÈ™Èy½?"iù"«"›?X={±0?X¶ˆ"ý"?†Mqä#¡?ƒ:pë'Ì?ïG"×&±´?†d-5Ÿ†?h$h§¶I?gÚDs¾8î?"	'冴?…"ž¡ÎîÑ?YL^?s0ïÛsok?u"y¦
G?TËZS¬ÿ?˜‰M
}U¼?rÌ?g€¹?ïS´²q#P?‰7Œó¾µ$?bi-^f¡?RÉ]µr}?"I<†"n-?‡¿£7ŠØL?îˆ3 †ø?©¬:nÜn»?r´ˆ+8ó?|ߥ4'?¥&<üEòd?¨
'™"¨?îÊ3œßþ?OΉ
a?rm×J\v?gçú¤á?¡ ïûÛ?‹°r4a×?í*ì±ÞMÂ?'Þ«ëc?ËI"< T?y}S˜þq?²uÈÐvX?'x"|®ƒ4AGN4FGL J1954.6-1122¿Æó7kb_ØÀ3 é_ªŠƒÀ8çDŽ¥JÀ;Õ¤xð¬¦@›jT1°@YgåÂg?ª—Àâ™ú?®¬Bn~R@±!«KrÅ@¨sÿ¬*¿Ã£]<Ç¿ä%"?]ä¿çšÁaߙ¿ã(ÛPN¿çd×Oݍå¿éÅW ºJAGNbll3FGL J1954.8-1122TXS 1951-115?ïö ú¶ë?wD+~¸§?ëÔvi.?øƒN—‹?Rݎþ˜?wF¦'s?ïñdØáqä?bßŠ=Rë?.4`ùmù~?>Ôð#E1œ?YoÂNÍ?`Xxû@ÿ?שׂ›5a?yëÜíŒL?[ÆՋô©?e²r^œ^?\U¸cŸ:?vd'´u ?ïí^:¦w¬?AYA;ýu]?6ìFÍóè¨?¹ü¸ê?_ˆy?ÛÁ??lø«-D?ïïD	ÞêË?rþ¤·å?+™÷º\V?®vDxø?^­DŒn?réÙåD€ù?ï͐±éqž?€AÇ­I•ó?H«–Ì«®á?]$½Qً?v"4#›U#?}f G'™½?ïyÔm]¯?'¸"EFÐ?bÁ	êùT^?d³qtÊ÷Ç?ŒÚ¢0= Ð?`/èz@?ïÎLFÞz?cv®6ÍZ?QŸòžRo?A€ˆp¡ï3?tr4Zµ?`ç½#A¡AGN4FGL J1954.9-5640¿À—ÁÄVÀ>ütÙÆ°SÀ: ó9H *À<`Ñ>K•*@ mIT1Ûo?ÿ*.!{zË?²yOa½	`¿¢kÁo Ÿ2?ñh'iIo¶@RÉÑoÊ?ïقˆŸ¿ÕŠûœ$¿åÕ¶`#× ¿Ú_á§Oe¿×LÕ[;ºì¿Ñ¿LF)¯ýAGNbll3FGL J1954.9-56401RXS J195503.1-564031?îÎÂÔ.¨?¦7Ah^?gï§J?lˆþ>{e"?¡£ÃǞ`?¤ª¡™aHA?ï³6lèOy?yü»u_??Qf§_›5?X"ï›á¾?Ñ	Æ?v²Ø#p‡?ï8pçɨU?†:¨QÖ'
?g{C!¥²¦?k2¸6¯=í?–znÕ?"è4ýеA?ï,çGU?tÆ´>w?q‰;	¹º¾?QúŠ>?¨M?™ØWªt?tkXþpÌ,?îYªD¦fö?£݂èØ:?puKÖøÃ?fKÎRèi
?¨V²;Âr?¢*ù×ÓÙ?ï+$­º?˜s™ÁíW?aSÚðz›?id±:4+C?›ð {am?—À%Sßk¯?îg"8F?"Omòoö?pTˆõßÏ	?m"ïÊØrÊ?§ƒMíg¯¹?"y$µ¸?í-¦çéfi?'†¶[ÿק?Šïб˜?sæ6ÂÓÍ?³@ÊÄùˆ†?'{Ýmš<vAGN4FGL J1955.1-1604?ïþY().À5%ð=]…À9¨èÄ3¡À<MjìÝä@ 2ót'Ý@8S 8"¬?²¼ùÅÿ(??_£Ê­à—?²~9|§›@éú8•Èª?ïoAT©P¿çPB7²ô´¿âI>¢Òþ?¿àÂkµZÀ@¿ßì.Ý
6Ê¿Éæf%ù¹ÀAGNbll3FGL J1955.0-16051RXS J195500.6-160328?ï«
JºA
?""^GS¾¨?KéÖSêÂS?SÇÚèuø
?ƒ~Ïû•·?'ºO?Úë±?ïã ùʱÀ?mO@õÒ?1)í'?<F(Æ?j¼!m?k¦÷l²×•?ïGÍÃë?Žß^IâL?eïgH
?u9Q'™ì?"Z(Ruû?Œ]á‰QµÆ?ïÓæ­¯·?ikž±ËÝk?XÍÒw+é'?9Î ¿4e?ŒñKýÇ{?h©:§ýP?ïx©‰ü˜—?•Ù÷TK5ý?_=™‡›­?aTøÆ?íú%à½?"T=ç8«:?ï°¤zÉí?'<ÖÜ+u¶?Cäzü—y?Qþ–d®÷?'š¦ö(¯¯?"4{¸Ø?~¹ïP?˜‹?z"Ø?qíȳ¡!_?|oÎåðÑ?£‰Îûo/_?–Ïÿ¿åÉù?îœÂûµ
?ˆwÊ3aΟ?qHÅáŠà?Yeh"Zì¾?¤
·ˆÕŽ?ˆ+HnAGN4FGL J1955.2+1358¿éÙº©è#ôÀAÞÑ·À9å½^šÀÀ;¶UNæíà@ÂІ×}@6ï›-îP?¸_ðU"?ÇhóÉæ¾f@
'¾}~°à@¸Wï«&?­3!8E'¿äŒKÓ=)V¿ä$"Ÿ^Õx¿æö`y½[@¿éœ#î¡¿áüŒéAGNfsrq3FGL J1955.1+135787GB 195252.4+135009?ï-ïhœæD?Œàry¢¶×?v9‹^æ›?ksÉÀÊ·?"³°ìpÞ?‰¾(Àm¸?ïZ•€bï?¡ÂÇæ3%?FqcÎ1x*?WCÃø]Œ]?ža"0‹Ëì? ™¤Xô¿®?ï!Pp?ˆ1 e?z€¥þ""?v°w[s°?•ÛµÜy?ƒ Ta»Œ?ï¬@'jî?bžS›".?G*!Úák/?,Àb±Žç?ƒ‡M¶r?aZVs?îe†
àG˜?œgÚ¥j˜?‡*H!"Á?'P)ʑý?£Ý¿:V?–ôÙù^Ó?í@PY¬6?µj"
Ÿ˜?Tmê†Ìƒk?fˆØä*´ü?µ«Å‡õ\'?µ>£ª™»
?î#"K²í?šn\ÏÅÃ?</Sž›?ŠFE>
˜.?¥¨Ç.ß-Ñ?"ÆÏD¼Á"?ï,aC"%?'jŸc­Ó?aÕQ©Œ1?OPOf¨Ï?¿É¼ÉŠÓ?ØœÄkAGN4FGL J1955.4+5132¿ì˜mŸA¤@'šoÅåÀ9†¸UFƒrÀ;ó€`°@m"M¥$g@çç†w~?¹Hw"^?¿†Ñ™»(@²¬ûv-"@õäÇ|¿ã¸×í'?2¿âüÕ©¿å›À¿èý,)Bï¿é'ìKî¿ïÿÿ&¦³AGNfsrqOV 591?ïî»GˆÖ?Qvs0B£?Aŧ'ÕD?5I
ߋ^´?Y¦-e»´?NÜÚR­AÁ?ïÍN¾e<+?ÊVú²i?IÑø_N3?XNs9`Yi?vaÈz‹??}·lžÿ×?ït]Bƒæ³?ƒA´Ó\?r°_¨4þ—?yKåOW%?‰í#?|½~CD?ï¹çFÂÿf?`¬*÷±4?Y»Mèýð/?98™Dosá?|‰)À0ó?_wºÐ¹©ú?ïÚbCü-?d-³±æŸ?Xön=–ª¤?Rõ¤'U6˜?i"…ª¾÷?^‹´U¾í¡?ï[™6?'9Z?_Râ[mz?s¯¨pÂJì?ŒHF÷Ž¬?¸È§ÜÏæ?ï
¨Ñ‰¹Á?Š"&áXZ?~…x¡]#?,^îýî?–© ñÔMˆ?…ŠE»6|ˆ?ï)ioҘ5?€žä¡¦œ?tÕJõD®¼?`#"U@ús?•N·¡?~&s"ô¯šAGN4FGL J1955.7+0214?¢tÌÝH-À*l´¿ÍhÀ:D÷m5ŽÀ<$@µÒµD@!F0¿:'ù?üïçžà*x?À«˜Ÿž–Y?·A©ÿ©&?ü\6@'¥LUC(¿Ù=ªðÙòO?ïû¨LºÃ¶¿Ð"yA4}¶¿âñÃA2Ð7¿ØßÁœ"[¿ØqMJ5®AGNbll3FGL J1955.9+0212NVSS J195547+021514?ïçU¨í¹?"4
•ýz6?b89‡''"?"˜âË¢ç\?ƒø0‹+Î?v§¨O½Ì
?ï'	óÒS?'òjïvÀ³?dÿ·±`Î`?kÅx|^çi?Š?ψDÛÈ?R‰ZtO9?ï'æ^¡Ô"?…d¢¹J[e?ll]8yÊð?eO'‰G™?—u¨Fš!?ƒÂ_—/~?ì
¤Úу?'Ãc"ëÐ?')ô³*@D?sç¯2O`û?ºÍ-°<sN?'¬ÈÚÖ¤?ïŸ'ïñ?',=yñ?uFŒ"û?vs¶gÑè?™ª¨é s?‰GHU¿?î›mâº'Œ?¥˜Mhcw¼?}Ô랃í?‡S+c?œ?¢§'4—úB?¢Ü"]Û¥?î,t8û¸â?•´WOa?zl'‡'*T?tÒtûc¿?©ë*>™£?"µP?™¯$?ç3€üÐܸ?¤PÝ÷¼?¡e"Œ¥rô?ŒUu'øF•?Îسj¦!?¤Þ"Ö~`àAGN4FGL J1956.1+0234?Ø"Í:ì÷ À*EóFí$À:Æ3\MÞ°À<8x{;à@ O¥ï?ÿÂÑ¡GãÄ?Ñd£Ã"ô?ÖW»þžV@FÚhµÌ@ó¹Qoß6¿ë7¯ß/j?ïõŠ@`B`?ߺl¢ë|æ¿Ø8ÝâHßî¿è¯¯…")¿áçÀÃÿõAGNbcu3FGL J1955.9+02122MASS J19562808+0234250?ï:,›-\H?Ÿ2ïL›½u?r¯~ *©?x('Å=úö?"Y?šì(£Á?ï"9Öîí<?Œ¹||ÂC?eZ±¿¼¬6?m§p}Þ«†?…ÚÝÂτ?ˆ"ÓÍk/?îm-ÕG¼ú?™M'h]´?ˆÁPè†ÙÒ?‡#‡‹?û?¢üÎp†'æ?•e,uA3?í\ҝ";?Ž¯s§jÞ2?e¥3FL—?r®´}‡?±l¶p®­—?‹5´á¬Ts?îtü'À?§/72î«?ˆ½M`­€1?ˆñ¿ƒ'š?¢€ê+o~ð?¢CÅÜä?îÞè]Rl? ì,ÌWU(?'+ÎQg"Ï?Žˆþ¹%r?›
')*?›(ܔ¬O?ìú/ÍDŽ?£§ÉT"¤4?"N£<ú?zUê>ãñ?³M½/óN? ò®&Ò#d?êdªañjD?¤Saš|
?˜ÁO2pª2?‹ââÈ¢÷?ÃU,'GTl?£È)H$'BAGN4FGL J1957.1-3231¿ß	áVÀ;7¼ä!}(À9üŒí¹¬À<? §?u@r⪯–†@–äÛ·K[?ºò¿¥œÝ?€{ ñbê?À—Á'R)n@	œp›ôgÆ¿ê b‹l¿Éy&‡~9¿ê$º"¦¿æÀ!ß&¡¿Ýsb"^úŒ¿ïçH®ÅzÉAGNfsrq3FGL J1957.0-3234PKS 1953-325?ïóäñ9‹?Ziü—Cí?(T@±b¯? '­yÝÒ?U,<?¿'5?Yhá[Ë:û?ïæ%É4´?hʙ'÷â¥?1Mš1âµ{?AíÛÞ!?gÂ&»^›?fM>¼D9¤?ï`7üý¨?‡w bY?hÇ<ëôÕ\?nº,Ü•?à5©<÷C?†&‰ô¹d‹?ïÓ¸[ьû?TùªÄðÑ?<Ž™<ùà?!¹ê@TL?tZñ´~õn?S.!1?ïå?|í'h?bº¼§*CÓ?8Øìßåè?1\N÷yÐ?gÀGé°«­?aµVò'?ïœ,|=p×?—3(Èâa¨?C Ä6Iiá?QÕjҝ ?‡ÂÔµÖ9~?–÷í°ô´Z?îê>³†«?'du|}?t´îã?j?x‡Ä#Õ6?‹GÅöÌ?z…ÿŸ71?ï‰MðB¯?r†PFä?U€-[Õ?CḲ+·?Šü´Ž@Ô?q\+äÝ'JAGN4FGL J1958.0-3845¿všªJGËÀ<öÄç%>À8P®{¨îÀ;«Ãæg@·RO@kÉÂbæ?£jåØÛ,?ÆÈ"D"š@"Ñ»IÊG@e:ÂHº¿Ït"çÙ´¿Ü¶}Àu%œ¿ä‹ÿG¶¿æ´Ka'bE¿ìO°â‹zó¿ê$Ɔ"ÄAGNfsrq3FGL J1958.0-3847PKS 1954-388?î{—‰?¨U…ŸeM?ž‰8<Ç?¤|Ý7ˆjc?žÇ‹ÝRÝÇ?•w›žÕ¹H?îüCN­Ò?£æÝåÁ?|KG¬‡ø?ŽÓa˜I®?—¹yõ±Æ?žtLý
Œ‰?é€[M6GB?´»Œ9ˆ?¼){[bsµ?«6'0?·Óª93":?¯ú÷®Rb?îé¼9V¸É?‡‡§SÁs'?ŠE1eè7?x?âèpØâ?•¥à*ËÑ<?{¨È~'ÿ?ìÐ4fË?³#ÔOàÙ?®á<6
TÍ?ªR
@¤©?¨!ÂÈg?¤àtƒm?íd²¹"?µ‹³"bŒ?œþ•É_Ã?¨'/=ÂG?«±Õ"!a%?­©}¾üèd?èxÑÚ?¹*Þ«›{?¾ápÙîº?©ã?ž>W?À‰gZµ¶¹?¶ª!¦=ÍÞ?í@ña׋?Ÿ64²s·? 'Bçu"?Ž1š'B0r?­Ù®µ°Ç?•ò&&¹±AGN4FGL J1958.1+2438?ëŒEâÒ•À8*»À9Â¥Ξ^À;î*ëf@!,çƒ1xH@[GA1M?»1±×(¿x}xü–'?¿Ñm_BÊo?û¢ÝŠµ%;¿ï'Yԇ¬1?ïÿ…¡•ž¿ÊÑÖâOj÷¿äWF¾*rš¿åŠ ½zIr¿ù[1e8ûAGNbcu3FGL J1958.1+2436NVSS J195800+243802?ä#r9>¡7?ƒÞò>Kj?pt#ÙR?d-Ë ííÏ?×wIM%ø?Œx‡-äÈ?ãÏ\Äô?É2æÃT9N?O‰â¸¸–?"ÃÂÑ»ö?×ä«¢ýèÆ?ȱò;!û?ã‡ÔÙÐÕ?´÷½/X¯°?—}äe'?Þu9?×x~zôÝ?´¨ëªG6¬?èMû,þÞ?¡|KB?4*Èä1"?)Øú2¿?Ê\BºÔk–?Ÿ0>m@M¸?ÚzH¾é<ù?Ãv§VÓ?ˆÚXl ç6?€}P@á´?â_r>¿a?ÙÎ	…1O?׏ñ
ò?ʱëüN*ì?€WkDDD?ŽLæ$Çž?ä6º©ßŒî?Ê}µy?ٞÀÕó'?¹UãBwL?¥Krvv'?—õËûiãá?áÜ:xaî?¸ìlXÑyñ?â4ýVòû?®Ã÷,›	H?¨Ê¸Ó4C?–|LJۯ}?Ø|®7œŠ¡?­"²ÁX±dMIXED4FGL J1958.1-0711¿ëÍeàžT®À2Œ?>À:¼áÑ@ÏÔÀ<SbI¡3Â@ +Ôíˇ@_…Q
8Î?Ç{×ómK?¨.ÀÃæ/†?㍷ä{õ@۟@!®&¿ã—ëy`>.¿è3¬jVµï¿ã†Å~ð¡¿Ó:Êi²K¿ãkùM^X¿à½ÛÍñûAGNbcu3FGL J1957.9-0712NVSS J195801-071348?ïÞa&Wúà?lÊà³ðË?1sËù¾x?.µºGÚ?op`‡¡–à?k1O<Úû?ïÖÏÆ`?rzßtc7?<õÃe}if?E'?÷&"?rÈÀÎé¾ê?qSٌô‰?ï¤zû–0P?w{3
í?P´(Ùðy3?;ñ‹~óµ«?"'òÅ?wK`/¦oñ?ÐgzÒ?in,'2½?C5ly÷üõ?'²ŠàzõÜ?Œ¡õÛ­?iHqq$
?ʧÙx?‡Ê&¨?D"äÅ4]?BBÜ|T°?†5»?†H-—óF?ïŠ.Mnâ?K|‡
p™?PFÌûøŒ?`"cÚ%i?‹k¢[!HV?
p[%ÎB?ï<ëș?‹PÂBã²ö?\ãJ~Z¤=?Wlƒ>>ü(?–¯máòÞ5?Š´µ—æŒ?îöWEó?ˆ=~&%Í?Z¾á<†?G¥¾8v`Â?¦Yò¥#~?‡ÞëᤛAGN4FGL J1958.3-3010¿¢%õº°)NÀ:È-œñ<ïÀ95íKÈUoÀ;Ùý2Æ&@ àZX?ý&ú@£^?¯ ö° Ï?˜ð|C6Oa?ì¿ÓÀí@
íœûù¶?ïïíJ.¿äÞv]Tní¿àR0N|e¿ÒžnÀ}¿ßœdпÕb¿¤(AGNbll3FGL J1958.2-30111RXS J195815.6-301119?ïõð5÷L—?DOˆ [Ƽ?P©œrØÇ?"䑪)-?RZ‰$⦓?Clº`ó¡9?ïåÕüe/ž?jh¯h!JR?4o=Å_Âå?Bæ3óù?gœ¿¥"3?g-Q°Ãu?ï™Võsù¼?y84*{=?W`Ù픿?Eï¹ß¨Ó9?†¾@°îp?x£¥X4	 ?ïnžˆŽ%ê?kõ4ǜ¾?T˜¼í	Aî?6¹­	£/?â£"ÚJ?k&²-Þ6?ïíq»Kº?S¦ÖÏH<Ü?/ýùaøì?#DÀV"?`Že'œó?Rƒ¢Ë=Hê?ï³VR-?ƒdï??F‡KiP?ò?TZpCFí?Ð5ÅNü?ÿoDÝé?ïN  
PU?ˆ'ZŽ¡+?`Pø…€9¤?c
KDÝa¾?"!Üëö*6?‡(˜þÓªî?TÌt?‡ßu¼‡¿®?k"E'÷`?S­¹ý‹]K?¥¤¹{iáN?†ø'.Ú89AGN4FGL J1959.0+3844?â@ȂÃÇÉ@%/<-­¸À9Ëx²Õ«À;'š0˜N@@q€»QO@1^aµ&¾?·¾Þ!³Ú?ÓUÃW@Ü
²p*@>3U—â	¿ÛW4ó&Ô¿äL#ú±¦¿çT¥ÿX:¿äô1•¤A"¿ïàñ4ˆs¿ïÿù³>†AGNbcu3FGL J1958.6+3844LQAC 299+038?íËn}â?­7´ß0¬º?‹$>´×ɼ?'§=œoÄ'?´u¶Qݯ?«cL:øÔ?êOvMP¦?¹_Vr"U?'zøfHÓ?_}}ªë?ĒÇɾáŽ?·Å¯Ÿ5?閍0]HŽ?¯ô'nÅ#?¥où?Ð??˜x^±GR}?ÄIÌî–Ý8?«nÄ8;¡:?ìdäàX´'?'fÖqèÚÝ?"¨£±-ã?s˜.Pæ?·®°6?Žœ&ýõؘ?êJ'
?¸XU°bh=?"kÚæãE×?­QÝBeÖ?ÄHD8$oÝ?¶úúøO?äÏÁ¤$·ð?È庫`Ê?¤Â'-ò?©ÿdαŠn?ÓÈ8ÄÓÀB?ÇO¾Š¥ñþ?æ"TÝÁ«?²Œœvð?­)G®¼q?œºP`z!?Îe¤Áã15?°²ô(nN¶?æÙ¯`w±_?§Q\·?¬=c
Ɔ?'DÒk<üð?͉éºæ'¾?¥~oÐÖAGN4FGL J1959.1-4247?àZÿ™ÂxÀ>ÚQÎÀ9]X «À<ä«ã£@÷8 ؽœ@(V£zÃë?µPNÅ_ñ?ŹH
°³@
Ár%·@ÆÈo(¿µVçÃH>³¿ÜMÍ=`Ó¿åªåò7Àa¿åÖmàXDæ¿ïS_²¿ïù7Y2¡=AGNfsrq3FGL J1959.1-4245PMN J1959-4246?ïI‰´U+?½üïn&=?]¬ôh'Ó'?UO¸QÑ!?"óú6ˆq?½«	nØ?ï辨Fۇ?hÜ!Õ
?6
§%ûh?Có–î¢B?d€ômüæ?e1ñål8?ïl¿»=ñ?‰4®>‰?~~QÀ@:@?®ñ%l?…èOr¥?}؂ÈOÅ$?ïôܵ;ûH?7è|‰6?&ºê%?
FQ˜\K?So7ûÙ҇?5ݙ<–M#?Ìln'?­·/ÛԖ_?lVºY»²?c*÷°'j?"Júmx?­ÆНs?ï¿Û;"DŠ?€ˆCA†{?EôM™ì?[LˆÀ=¨C?}SÞ¥Å}t?~¯—1àLÜ?ï8Úçí?Á¡ùÏ	I?‰](0=
?ˆ‰ÙòŸü'?'ŠP"zÍz?"Æ;é.:"?ïå*xñе?UŠš¥>²¨?;öY>kwc?0/%VÑÁ?gV»©[ÿë?Scæ¸ëAGN4FGL J1959.7-4725?ïîÆÁ½F"À>Ø},{‰
À9!´:.Ï÷À;¿"(fQ@S±uƒdÏ?ù{üä?®Õ¼þ ?ÀqW†#Æ@À­Ù©@ö"Åš)¿Û¾P§ET?ñ³6#¿ÔÊ¿ÁÌh¤¿Ðï»dD£¿ß†—D¿ã|}`þÈAGNbll3FGL J1959.8-47251RXS J195945.8-472531?ïAÈbb~X?‹îz\íŠÀ?'X¡ìù6é?~Gí¿µ†æ?5EmX¯*?'Ð"‡\\?î©Ç¶QO?¨™ù¯Ò?Œã@E"2n?š™°R´&?œUi¤gó?žÿ{Ûè?ë±fñÀeû?¨`hU6D?©d¸5N?ŸI$\á¹?µÂyíÄ΃?£ԟ¯&?ë=[)5GN?HèÌéšf? >¨T³ã?€FâIW(-?½õÒª‡Rš?›eßxŽ´?힏»µ?¦Ì)4ÐÄ?›Í.Õ'$·?—ʽŠø¸?¨8/š˜	[?žúZ}
Ã?ëT‰¥ìÊT?Å'³Òn¼?°Ä?šh¯>?Á'åràó?´—s5Ã
 ?±‡Ùo?éàîPf[?¯+‡É0·¸?®•ØAeŸ? ~'ƒi»â?ÀÖЭh>¿?©ç%êOˆŒ?è3·ù'9?®±çr"E¹?¨µ¤\Ù.a?"(%™?ɉÈ
›9'?®õdÓ`²AGN4FGL J2000.0+4214¿á.ÇÌÿ#@ÉéÍ³}À:-ÏZsÀ;¨ÕÑXLÈ@îd¥q>@]_V§­?Ãà™~욿 ]æ»?ÜŠ]ÜT@eLÚÏ¿ä×MÄ®ñ¿çûÃà•®¿èKÈö~vþ¿ä-RòK¿æ‹È ˜;v¿ïC¬ýúlAGNbcu3FGL J2000.1+4212MG4 J195957+4213?ï´pV÷ö?w[TP@ŠŒ?:ýuY Ê?0ŽÇÿ?'þŸƒ'?wùãòˆg?î©Ç1,rÐ?«6ª€?Nî˜hą?`è!›"ô?¤ëI1É?ª™<*qN?íϬ">#ã?Ÿ~;¦;–ï?x{¿]]\1?v˜Œ®Å"æ?¯õ¿ÑõÄ?õŸ_ô_Í?@rÙ?fë~…˜?3LYne?¸ãÛ#nŠ?‡á5y.v'?eÚüw¡­}?ïp2(àãŸ?ŒKx%Ó?E‡õ9g?@Ûö¥×?'M~d¿/F?‹ÊÙüŒã;?ìÉó½…?¼C©"ë"?b¢Ó²J¼¦?€%ssìi&?¹"¹ÄU†¥?»"Õ¬Jì?ì0R
Ÿý?¥j§2œOû?ˆç—%Ý?"–%#ƒ›^?»bñ¸zÁx?¤S|^2Uâ?îÕÖbð°?†m
Jå?LCð낱'?;dª-Č??¢1Šo
`?†*O[sHkAGN4FGL J2000.0+6508¿êŒ:
'Ö@1ªDØw$ûÀ6ï.¾YlƒÀ:é">¿@¸L]{±&?ü.ˆ>''ü?mJ—do?›°]ÓùE@Ô>š4@*æ';Ù?È˜=V«¿Ó¬%Ã'í¿ÚÄLÉÝ.¿Ùt-݈ݿà¯ÁÏÖ¿Ó_\òI^AGNbll3FGL J2000.0+65091ES 1959+650?ïí½mçÂ¥?` ;©?&^픚Xã?ÐÂñóË?`Ü£ËÐØ?_·çOìdµ?ïÙåóÿœ?s…Û4cEà?C*Jæ£g?OE¶†e±?p§¼š?#ß?q©¯~lÉU?îW(€|½?Ÿy;=3`V?s?RÄ{Y?'
‹w ¬¡?¨%¥'ìÉ?ž3ßÊc8?ïô̔²më?CÌVÊXA?;KD‹>÷/jÛy,?U¶´WÄ
Ô?C‰½"yø?ïÓ¶Þ£äÌ?t0ªV#!ì?3ƒ®ª8‡=?+‡S¤/ì?tìUÕÔÆ1?sÓ8{L?ïœ÷l³‡?Íäéýt?Sûq1ëµ?b±‹<¦[?†B¶¤e|;?0ZQ4o?îOxgß|? ÝN9ÉÐC?m'‡Þ ÿ¨?z#Mtîc?©.ÿûUÿÄ? ¶GoM?ïì$ˆþA?XøkÀ§'?òŠMÉÌê?ٙÅ'ü?c<VEz"6?WœQÑ?%AGN4FGL J2000.3-2930?çILWÏþÀ:þó¡LìBÀ9x>£©½ÔÀ;ýû›ût@>Kw1@‡ª4ò?²+g¯fµ?ªž,a™`?ôYè'u¹?øh5Uø/&¿ÙíÚ£úñx¿áf½+-«¿æª°þ:-"¿æ|ZYê
¿èþ»ýq°G¿Þ	5]ÚѝAGNfsrq3FGL J2000.4-2926PMN J2000-2931?ï'vÛë?'Ïê8ÆÛ?kòìSHO?fõ?M˜ó*?—'ÇÉX?41ib"?í߃¯á?©«næ?™«uå	"Ž?›éÀ¾ð—â?¥2h0£³?ŸTÙúqp'?ìîn(^'?¡ÿMj¦mç?š %ù¤Š?'ÇC~'=?±ä…?v`Ð?œ¾ßz§?í0co2Š8?¯L¦z<W?¡øÆK†¬?ƒq'†s€?«ÁGÕÏ?…cF!²?ì[Ç=/¥#?³6!Aq¤?[ö_"•?ƒuKèÕüª?¹vGJsµ?²jꙤFë?êWREáÐY?Ár/ÁÓcY?¯Çö7%?µGŒ@‰•½?½ar²`K+?µÝä»ð U?ê1Ut?†Â?¬lÝ;ƒ?¦B[6Šë&?™Š°ø¤Ïª?Áª`O¯?§ÜßTéÛ3?éHïþ*<ê?¨F†ôu?·(ç	? }Æûã¡â?¾³Wþ3 ?ž¿jD´"ZAGN4FGL J2000.6-1328¿ïÿeÙ§ÀÀ5QÇ5ï¦À9Ãí~<QÀ;ý}K…9@ø‡Ô3@ÝS¨Á?·»júŸÃÕ?µ=ä7
?ùš£Ÿ¬Ù@ózÜÀ
¿Õ·"ÁÄO¿à®È4·—±¿è (ÿӊV¿èÓ}æOU¿Üöÿ<
È¿è<ýâC'AGNfsrqTXS 1957-135?ïÚíÒ+'?i/ÕG%®?B<¹»²?9ôvdž?pF"!¯L?gG%P˜"?ïÅk
©Àó?{¯k_Ãã±?NXKé‡?Y ¬·÷a?yxºCòl?x·=Ք?ï³VÚi?Ôfc•¶?jBvݵ?sˆlci%š?˜áC'5?@ì
S?ïdeHT?jr	/p/d?b™û‹ž{£?F)7Þ§Á1?'*ÛÇ??h.Ïoæ?ï¤é:Zˆ¦?|sºSÒ?Ušas@-?PQ'÷Í]?"e9íðß?},»-Ò?ïOÅz}?™
åZü?gî0Où‹?zÿm,‰ð?"	Š¸î-!?"%([þSd?î'úÉ
Í?­>¹ˆ?{¶æ]ÕÝ?}žDµ¥?ª	v­M®ô?›žU4¹µ?î ÷å\ï"?Œc$¸R3­?9\8¬A?k*¿fÆâ?ª	^žRZ?‰è^NéAGN4FGL J2000.9-1748?۞QêƒlÀ7çF˖lÀ8®Í"]"À;˶…ì>@Äm/ƒPW@
4†ðIª?¤®ª¢ÖY>?½[¦Õþ`?÷jÈ˶LX@P¨dÅ?ïÁcâþ¿àØÙ`ð¿åú%Ëk£½¿á4&­é²·¿èy4j¤9¿Öð-¤þ҃AGNfsrq3FGL J2001.0-1750PKS 1958-179?ïõQþÐU?Bò*ñ¨?$"sÛ"û?žÜ¸lä'?R׳Â"†?A¡î§™?ï붞b+?ho"Ûcœ?3SöË\þV?Di¦|l2Š?aÒÊÌÇ5`?dü9$x€%?ï¦q3ý?{Ý15
…‹?Y5çwƒÔ?_'0R!ò®?ƒ\3÷B0?z(ÜÈæ^Ô?ïßU2Œo:?OèP2
žJ?KD+Âá\?1³°,m?iÙÂr6™f?KëìÞÅ?ïêÌ¡¦$å?T¼(FgK?4oEŽH8?&¸7ghØ?b¥z˜¸v;?Sgju|Gf?ï¿3j¡Åž?ƒäü
Ö\h?Gnœ¡XÙ?^Õ*+=??}"¼ÌÔKs?'fé2ð?ïb®ËQo?†Ã{ß,Gr?eO牒–•?g‡$¦m?')žôr9?…8x‡õ.?ï®ï'Û ‹?lâà¶H?bnB]ߍ{?Pðí¼ÿÜ?Qh¿SŠ?hxÖäÔY¢AGN4FGL J2001.2+4353¿ë—ô™Ö'ƒ@t3ÿ
zÀ8É16Ù±À;7ì]‹ÌQ@‹7Ö[û?üùä"rÁ?¢¼'Ÿ<ø?¸ÄP@N¡@«â´•žb@"7Ð%¿Ýù7Ēk¨¿ÚRðÛö¿Ö2ü´›þ¿Û!ŠßlŒ›¿â¸oG¶¿áö˜ã'4pAGNbll3FGL J2001.1+4352MG4 J200112+4352?ïÊ1ú£õ"?f4ðöµ?OÜïD`c{?F£´µû"²?vëd±Hï?c'™ø¾ˆ?ï–Ägé?'抇.½@?JKR—Rd?cmC"¢@?ˆª1èk?'LÉ(ÊÆÛ?ï)䘤Þ?'AítÝق?y<m' Œ?"-|µ¿1\?"tQ¬22?Ð단?ïã¯pfM?RzŲÀöÅ?Èjœtõs?×.ûíIy?kŠpZÇ?R/ԝÀ^™?ï¦1=B^R?t!$‰íj)?M,$ìÙµÉ?D\ÁŸŽ¥q?" îp¸.B?sW¸¨Çl¸?îòýuâl?¨ˆ
âäÉ?b^(f'çg?"	ÀW¥V²?ŸTŒ6i$…?§Í7²S7?îÄTE|‹í?™3¹^é–ó?x­"b›Åµ?TìòÙ:<? ¥IÙÿ?—/©÷ñÏÍ?ァj_Ô?oœ€ôC¶?)Etß?2òÝãä?€1DH?oEæ¿G—AGN4FGL J2001.5-0818¿×i~–*p¹À3TFù¹"âÀ:Ш·CΌÀ<B
Ìsá@žŸä@OÒ}浬?Ä2"ý[
¿™f`ݐ?ىVá
K˜@Àû*XC8?äzfކ]¨¿å®‰J–ý¿ä{Ëóˆù8¿âÀ_C‡i¿Øyx;ûÙ«¿Ûƒ½D³«AGNbcuPMN J2001-0820?ïؘ»€Ó?³@$ôO´?…·dj>¶j?³=k]Ãh?t¤ê±•]þ?t¥YnmàE?ïÄGÁ×ô?vÒl#2ÂÇ?K͓ÿ«?S‰»»-?zz)'Ñ£~?tÈ^¿C
?ïH)ºc"?€5'¾ÿ?TE¡8ßy?[a)ÔýUP?‰eA[³1?ÃjÓ$?Þr*"?dlEº%«?:ƒÛwØW?!‰ñê"?Š}©–?[°?dKã8¸?ï•.Û:_?ƒö±<ðk£?Uªø s?gåý	¿?‡þê$x9µ?§hŽÝ?ïx"®·Ò®?"C>Õ9-?T£Ù¸tì?j=2—ô?F™&%´?"°ý…`Ù?ﳈƒÔ?šºª+$U?a·æ½	€?iu†7Â?šò'NP?Žñ­rbŸ½?îˆÊçšX†?"92†§ï?TÎ'ª"k?CõV¦?¦ÌàØmJù?">¾!#iNAGN4FGL J2001.7+7040¿íûœyP€@3õXÙµé[À:Ÿð˯–À<Mҍ.#@ùX…Ó8@ó:G#«?¸F	¤™|é?¯ãʝÑc?öGŬGH@.çÉþ;?×¼ÙûŸa¿È
‰*‹™Ò¿á7'Ô'½¿âa‡"à¿á`žü/¿çŒ:€¯gâAGNbll3FGL J2001.8+7041TXS 2001+705?ï¾ôCM ‰?eçsoJÿð?V:p3W¼ô?Aâ
ꦩ?z÷B7ü$b?clü…´£Î?ï¹.ú?xç*7_"?[¹I‹"ðû?fä»F3¶?|ˆ&ßE.?r˜PÉe?ï•úõ÷_ë?rM\p1?`…j6¤\¹?Zìbå ?†_çæ'5?oÚwˆ?îûIÈ~'
?týf8<?€¯Ì£•?YQOd'ƒ
?˜†ïý$ð?rÄSuب-?ïyUŸw\¶?|gŽï6?hW¾(?UñîC»ÓÃ?‹"Ðøy¥"?xʓB¯«h?ï:È³–#?'Ð4'¨O:?l8‹y%ÉÔ?uwÙÄ·?•'5u™x?U«´øeo?ï(A4et?…|ÉÚHD?n¡Buêi ?e~ h"Œ¿?—#´²q#P?ƒ;*²Šô?í<¨–¦d?~áh'xÕ?–dˆ`yKø?x?'ž³?±"ø¡âŸd?Ž¢¿ÚŒX1AGN4FGL J2001.9-5737?ê-/|ߎÀ?÷ë[-M@À:‹¹ÝÀ<Œà«¦âW@ðDK3…?ÿÙGÏ¢j#?Á·vÙ%K?¶W´ü?öB;C¢ìÿ?ñ>¹Ôw'?ïùPMö-¿Ô]Oö¸Y¿åP
nîË$¿×[l7`¿]¿Ûû+ÚÏCõ¿ïÿÿÊPËAGNbcu1RXS J200205.7-573644?ï¡IëVj?ØóMo?XÝ°[
S?VÒo/ÙþŒ?"'	}8W8?}F2;«ð'?ï.kçô_R?'2ñ;czÆ?wM~Ç?x<4Gà?"k/™¿£?‹ý0"ú¯H?îþ5½§?Žß­þj#–?v`¶ÎY¦ý?z"1¯'À‹?š¡•£,û?‹…?GþR?íX<ÿ²Ã?‹\:KQù?š\ÃRå%?zwsØd½?­MÎZšG?†ˆ÷µÙ–4?ïkû'̺?…Ú‡¢*Ÿ¬?h/—áX?aÖkÜèé?Žõ5`Yèò?"‰'8Č?퇄·<ö3?¬†{&#ú?±P·«çö?"¶æü½Ï?¯/3ÊDÎ?¦§uü
Ææ?î´ÇV?•·9H•?O¡_?°È"È?£¤y
l¾?'·©Ïòœ?饈ÌS"?¢»ª'ÀÀ"?®á? ~æ?–ehô?Á±Œæ"k?Ÿ:·ʺ«AGN4FGL J2002.4-7119¿ï"Té'À?@®û*®)À:Ë«®o´À<'°P$Ü@!ªñ§L‹?ùèäZˆ?Äþ2J€ì?¼"Ôeh±?÷r¦É¢@#'+f5?ïÿÁìžú,¿îÆŽÜ&?ÞSÇÝúœ"¿È1q'"[¿Üƈåí/C¿ÏpÜÔ+çAGNbcuSUMSS J200227-711940?ï¡-«E#Ý?†r~D Ý?3É'®é?-Ñß3äwž?‡öìáQ?†GF,ãw"?ï ñuu?+xÿC5@?VS¡4ï|?^c¿FÀ?"ùZ©¬§·?~‡1xÐ!?îQ'Ö?ž¹P>û®?Z¡yN­Ý}?Yzš:ªQ?­Is>§9?žÇÒ*ôd/?îëXå0?ä`öaõ?a=HÀx'œ?I
S¯lL)?¦Ô,½xF
?¤ä? úð?ï,"êÍÀ?"‰:¯\;?BÍvúâü?=—…ž·$?™ÖöíÚ§?"WØP…öÇ?îù_'&?œ³–•º.=?dm"ÚOê?r×ê÷S?žNpcZçY?šÎlæž?ìÙDCÉ$ï?¥ahÚòÅÔ?a9Î,?bd=PÊF*?¸¬p%ûê?¥]†Â1É?ë÷"¶/É¿?–Å/È»?q¦¼uí_?d¥œ[cÔ?¿,~‰Ùï0?œÎ"Žˆ
AGN4FGL J2002.6+6302¿×"öÃp@0q€²BÀ;qPþU0À<Ô®¥šXÜ@""¸;›6¨?÷¤G¨5=Ï?Ðg¼'c?ÐWˆ
€@=Óºý—p?÷ÙÙò$J¿í4DÀ¤Jx¿ïÿê o·?ð¿Ç—…BI¦'¿ÛåœFó¿ozFm!ÁAGNbll3FGL J2002.7+63031RXS J200245.4+630226?îxÖ³€u†?«+À
¦Ð?T¿=P?Xššçó•?§Ìšáç?ªÖ™*8+Î?îwÔóaáò?©"'Ÿ)0?'‹¯À´Oý?…¹,a%íw?£ßÄÞ,JÖ?§À®'è?ëÇb«#V?­=cF?r՘£O?vD~¾X·?ÀKȏj/?¬øÙG¾âR?ì6#è^ðô?˜%·ØE'6?€¤"&£?mô-1m*?¼M<C¾?—ÜÔ¥àÚ?í³o¢5…¯?µ ŗÃ8v?_gæñt¢˜?^µ6ƒOv?±æãS'î|?µøJ˜ÄK?ìn›AP?¾t÷t|dç?–'ÜIß y?£š_Öîþ?¹sÔ&`?»ÐÔ÷R?êÀìA1M«?±Á¬|-²?~š©ÖÔì?€¹ZálPê?ÄR%‰î?± |b¬;•?æ깡?°Ä|.&?•.ýxÏ?ˆ|,vUœÀ?Ò終§8?°±ÍÝý½AGN4FGL J2005.1+7003¿æ+`Ío@3oÚè'®À9ðhÒQqÀ<#ñLÞÕä@ z¾©HŽ9?ú;o&ÿHJ?ºÀˌ°Ó?Å®6Jü@ÍÀ:S@ð6¿ãXò?Mé¿ÃþFïƒÜ¿ÑÂQž®+w¿Ð:² {¿ßGC…:è¿ä¢ Æ´…AGNbll3FGL J2004.8+70031RXS J200504.0+700445?ï܋i*;?§¯ƒêXÏ?ax$ðøj¨?–€Q_sL?aüqë«»T?˜ßñ´ç—?ïԖ8wQ?x&C͓}í?N×^ö3A	?[qTç¦?qÙ÷քgI?s
b6…gþ?ï¨Õƽáo?{â ×ý½?e°}õ{Ë?kîa•ã?€^oš	Q?wús§3¨?ï¶35êü?q¢³;Ë·?fê™ÊŠ—?HÁ"YhŒÚ?œ‹æcÝÜ%?p®ÂŠþp?ï쐊H»?U´ÅÜýù>?Wò‹fš?Q!Vͦ@?PÜì¥R¸?B3]•Ì™?ï|"ãH܊?"6
)ÙÖ?aÙÞê™Ùá?p.ÐÒÕ?ŒdO}Dð?'Øi\;Ên?ïcÎޗFû?…ÿUŋ8N?vpf/4ý?zë G?‹ÔCóš£?4þ}‰™¢?í{z6tR°?Œ×€@=n?z¬òmÄtQ?emĝä
?²y_$Ü5ÿ?‹ƒÙnßAGN4FGL J2005.2-1822?Ô#šyðÃÀ8Gà·õ¥À:YEnŸÀ<o㽪@´"¢lQ@ÜòB9`?À¡âhjx?0°[@+kÇú*(¿ÛŸ¯È°š¿çèµ`Ÿ}¿ê@bUµ"¿â
r_C¿îØð²È?çý/Á
ÑÐAGNfsrqPKS 2002-185?ïÄߤڄ4?"&´ÇŠÕ?PÝÄÕÞu?R­ÂÐ?yXëû¥v?ƒŠ§Œ—¿?ïÊ¥dËS?tñ~¸b̚?Iâ¿:Óµ?R%íÂ<-^?wŒñ`š†?rŒ4ªÏE?ï6ùr-€'?-¨ïG×ø?h—M‰‰?pH¦Cjn?–
ïß)°?‹ÒÃв‡?ï©«"¨O%?bôÓ\?JnŽªZŽ?2>™ Æå?ƒóä30Üÿ?bŠÐM'?'‰v?Š¤÷Üö¶?f¶åøŸ?fxKL£×i?‡¨öEüjs?ˆw¸Rª7p?ïmì|Àoò?›ïñPK?T"ã$¼·?eßJ±f?ù226›ä?'¦‡Õ?îqÜDu6?›B¾9¸½´?vP#J?{šÞ¡Gx?¦I«Àn¸?™…¶áô"L?îã= ¿4«?ƒÁÇ©­þø?gª®­?Yy¦0j#à? QŒ®‡cø?'r¢';gAGN4FGL J2005.5+7752¿ëÛ¿*2Œ@6»½¯ljÀ8cSÒåë'À;ºåaïa@>®ïl4@"]ªÖ?œãàBSX?ª[<D\"@
ßE™›@¿ž$DÙ¿ÅN	¸»rÝ¿à'úáˆÁ¿ã¼Lßx÷¿á{¸<òϖ¿æÄÕA»a@¿åA".ÎI¥AGNbll3FGL J2005.2+7752S5 2007+77?ïñft©I?JòªÞ>"À?3ùÔð?#r¶¼)G?XqPrÓÖ?H¾ê™"Æ?ï֊ìÆT?v8--á?J1®uëé¡?ZC½\%ø?qtT[Ê­?qÐóÂÈN?ïº38wÑÚ?r-ËUV†8?Z·¸¦»|?\ÍÇ5¡2?|8u—"È4?p¨¦SÈ?ïðÊáu?Aü{™¼\?3™µýÈ¿Ê?5Ãd·?Zùþ")L.?@cý°|Èä?ï䒭'|,?]GÑÈ.?8ý<òz"L?)J×o3-Æ?hM«T»å?[è3‡£AH?a†z%?ˆ3ìÞ¾{v?Y…î-g§?jËru!?‡féÊݪ?"é`P¹k?ïy¶#Vá?…[ì²<Ë?f±=Ha¢ð?jekƒÍz«?Œ
CSo?ƒ¾.õùy?ïÚ:çk?`5¨ù|>?GÔr-F8Ü?:äŸHõ¨?oÐÈQ·[?\ÕÐ[i‰AGN4FGL J2005.8+6424¿ï8L
Zíž@0Å:æ…ÛwÀ:f™5ƋjÀ<7w^@1a¼­ž@†ö¼Š_j?Á%x	¦ó?ÏWá&öå@b[T‹@Ձ†R?ïòJ¶Ýw¿ÌÞXeqÉÇ¿åêûVM¯¿ãG¦¢–˜]¿ëÔ@ßn:¿ïùö€û=#AGNfsrq87GB 200541.3+641601?ïNõÄÆK²?¹†ó½?ŠZ«Tÿw?iè•{?çã'\˜]?"ð®àDý?ïuÛ0_:Å?'ŸrjŽeÊ?pŸåúJ}?x7¾ø–±µ?Š{ãõ4)e?Œ+d}p'·?îtè‡	ì_?—.U["¾Ÿ?–·œ[bHÂ?¾Ë}ÜM?š«RÃ`+S?åå³´´
?ç_}È?€‹AH"ýV?‡#…¦¦?hâ)áëäà?œúâ‰Ís¼?}ޙ#-ç?î«žÃ"Ø?¢;mIœ¡?¥@€ŽH?"¦Eä
¸?'*"«#nj?Œî'ÖmÇ?î•"‰×?¤¨'¿f¤þ?…%{L˜B?'²/®¢?¡^¯a!Æ?žBŒpG?í*éAïÛè?¢%‰ìò>ô?¦ ]&?›+Q×À?§1Z†'gX?"è6«OÞì?ë™H'$öÉ?î®$ê:ß?¥«A˜`ñ?Žº<«.i?¸`ATK@?šd3'ÂEAGN4FGL J2005.9-2309?ïžØE%ùåÀ:#'ˆÀ9 Á¶UaÀ;Þ{ÍÖ¸@HñS¿Å¨@19ÓÀÝ?¯XËH=[€?¹"IV
N@<êy…ýÛ@b¥ç…µ·¿ÕÅqú_r¿á.›‰]â3¿æô÷ŽAvÿçÌ.¬­¿æm¸¸ÇÝ¿ïÿülòAGNfsrq3FGL J2006.0-2311TXS 2002-233?ïúÝܔ•ú?@Åéñj?Amg:Ó?ú¥l&'t?B`_'•?>ëÏ'5E'?ïï¬ÖbLÑ?b6™g@?(–¼¯e?7"bÿ?]"j'Ë?`Wƒdmü©?"÷öò?y™¤L7?\ÈçP¸Õv?LOÕ óåq?ƒúAèR·?x´>S>?ïøY0ÙøÁ?1‰^ývd	?ù›'›?E†"ñ?K\	Énj;?0ƒeˆ?ïõ[J‡?R‹ÝßeËø?¼T¤Û"?G˜o¦?Só"‰ù{Ê?RõlªÝ?ïÌg=7)H?|Êmax²?BÔóBW"?X"RR">¿?wqÃ`®²?zþÓN¡ò?ï[ƒ}ù^?…}HÆÄ?fò
Žö3?dàý,ý>N?'±Y¦Oå?"KÛ¸²jt?ïî\y?Mš™¼Y®?/]÷mß •? u>UÔRµ?_[OE]Œ?KßaüýAGN4FGL J2007.2-1433¿íê›÷³"À79~ºñ6À:TÌ4 ˜ýÀ<'¬-ðÔ@åÅj­É@¦rÅð9¹?̍ÒfÛ)?è% }ä\`@lûï¯P?ûœNOnRC¿à
sáÏw¿Ýe~_–~¿æÁ³"¢Ú¿ï¹û8ðâ¿ËÁßeUÅ¿ïÿþBe«+AGNbcuNVSS J200711-143205?ää_øp?ÇÇøôëFW?Ëtõ™¾5?Ã;šU+U™?Àùm…È	?·ã›aVu?æ0{MSDö?ÐÍR6aD?˪K½Ÿñ?Ë!³Äh$W?·'ŽìMf?µ D/d.™?áT[¿f?´d©"À÷?ÑP»
³?²Ӄ§I?È«Dxç?«Kàn¹Gê?ÜLkÍrRó?¶]Z"óˆ?Ó$µÁîLy?¸Ã—SuV?ЎÞpŸ`"?¯s}ÿsãÞ?ؑª¥Ž" ?Ƕ²#~4c?ÖXñ^ã¡a?ÆDø}ç?ÑcûŽ<?ÄyfÞ±PÅ?×ÂÀlÊ·&?ÒÝ|pF—?ßí®Þi?Ò»ÑØØ?Âl£È­¿}?»Ù)äR?Üɂ•qí?µL§"«Û?Õ"ÂÕ¢O?µ†9"Iêô?Ì'u*à‰?¬àÑk¶ë?¼0""vç_?ª4b×<r?àƒ>P§E?ňâê<ì'?×íz¹¦÷?ÁÔH¨KŸLMIXED4FGL J2007.2+6607?Ó]H¥¶2'@1s›fù3]À9Ò"ÿ‰;À;ñgº#|Ý@¢
¢Ed¹@]e¼{a?¿2ŸÝoK?÷9½ï§@'¬'\f@lÐ"l¼l?²2³=ځ¿çòêmDŽ¿èÖÁ½Ð»¿è7çÍÚ¿ð?ïÿþR€ÖTAGNfsrq3FGL J2007.3+6605TXS 2007+659?ïßɽ‰ôò?h,K>Ãd?cÔ£¬R8ô?b/Añ!K?XÃ=u5?TÞEˆ9?ﻜåÃ,ª?…}v"E+?[­/K­Ó?gÄI¿˜?{FA-HïÒ?‰-¡‡ÿZ?ïGkс´Ã?ŒÞBÈ|†?ƒ)C7蚣?†U'ß?ŠûÈX‹ìº?' fÊàɏ?ïªfÒ-E?f±ÖžR&?a	c}<9—?FôPê"6?#ò‡ù1z?cóÞt@ù?ïÁM†àHC?tâµTBE?vEF¿Ú±t?qän3wAN?b'ë|FiÊ?]1Xœ2(?ïKM-°<s?›\)"Ж?sþI"ËÜ®?‹Ë|¶LW?'–Çð(£a?'·ÇŽÒË?î­wZ]!L?–ï{Vl?'x`³?Ž™·V?˜Ù˜ŒÖ?Š­ÜŽåO?î®ûñÜ?‹ëd|&?É¤QÓk?nåô#Èn? ×Ú±Œ¶?‡<^(uCAGN4FGL J2007.3-7728¿êhSjOÀ>†yF<û3À:k‹dL°³À<G¥«ö"p@.ß/ûÆ@F5~g?ÄxH:	ç?×±0@KA¿½ð'@¨žÑç¾Á?ï¿5¾§¿Ù€_ víó¿âûH
ZÍ¿èÙéëÁ"š¿ïþâßâÍ?¯aT¿Ü	½AGNbcu3FGL J2007.7-7728PKS 2000-776?îíÄ£!q"?"öòÇ¿'?‡à8Ôä?æ$¤š¯?–Wi†Fú'?qK›+a?ï{CÔQb?…NJ8jº?e€Tûb=?m@s¨cIó?†Á»=j?€ÅãR¸ó?ë3ÑÜ´©ô?©›igøŒÄ?²z³÷•ƒ?¡x^é¡B?³çieõ'_?¢XdÿŠÄ}?ïe™D_*ˆ?m‡^þšÿ?i¼êt^?NHòÖ?VŸ-?kƜN°2?îU¬Žá&?¡Îðe¸¨?'˜g50rë?'Α"¨ÎG?¡ca™åÿ*?—]¹öY®µ?îäNkm?ªtkŠ-9 ?€ø'yÇó›?'ßSô/""?¡ã–yê×Ä?¢ðźߺe?èþìŽLù?°{jÿéŠ?¼;ör¯í?¦ºAfÊê?¼_—%‡4?¥ÄÞßÒk¦?î­CD£H?áñk…?'nÓÉök?k°NðV?©ùvÛËå"?ŒéôôàÇhAGN4FGL J2007.9-4432¿í´Eñ•ÐÀ?ؖþ´¦eÀ9tÓäCÀ<€§ZL}@k›@½Òtw?³–Ç'5#ù?ÀÖ­ _@%çñ@ccK©Ì˜¿Ù/-••¿ã™*]÷'¿çèÎUcä¿ë¼[ed¿æŠX^©¿ïÿÉC«P{AGNnlsy13FGL J2007.8-4429PKS 2004-447?ïøéÌ?'Ä?Cÿý6¼#?+qÖýγ?5ÞÐ×AV.?E|†Mp£?<þ"k?'µ?ïÝ3Ѓª?qc¬·‰Ú?:'bˆÝܔ?EÀ¼ƒ'k?ozÐú©?osjPðÏ1?ï›™ì©?zóuq?_ôת	Í?`O"(E¸T?…?~"²E?yIâ¶fÙ|?ïÜH"—îŽ?P-f˱æ•?FBäSàÐ?-'ÝÖcÇ?n&Âl¦(?M:œk—ž?ïñ2ÇnE?U½ì\!¥?5üÑy›|?1—M[ð
^?X=ÈoS?RàK+
éh?h_K?HÎG?R¿î?b¸|ñà²ÿ?‹6±áÇ­??‹ªRBzË?ï4Hòb2¥?‰õ©9õš ?jƒ€2¬Xñ?d£cuù?–&qµ£03?‰WÍs;Ü?ï¡åa²ç7?o|'qò?^ª*'?J±@ŒÕ¹š?ƒÆŒÒáb?lšf¬àíAGN4FGL J2009.4-4849?·ú5'…XÀ@M!…Æ~À8.C~ÚÑrÀ;g1Ԏb.@pÁñÒk?ûü݆Xt5?ŸÌØؖ&?¤"^$Bú@é%»{k±@(ýâPm?×¹ø^ËèK¿Ö€A#5å¿ÚÑMD×J¿Øj¦sG¿á·zö@c¿Ð‡á@!X?AGNBLL3FGL J2009.3-4849PKS 2005-489?ï÷'"ì'J?@ÀaJ_œ?Ž8'åKÎ?æ¿ÌséŠ?Od%Sf3??³;²ÑO?ïè¢ó¬×Ü?f|Hóæ"?11GÁëÌ?>×e	@Õ?e6ãB
`´?dEnÁ-ì?ï"Ï'šù–?"ØR«?dKÿÉ؈c?t±®N6\?…ù60j`Y?kL ì?ïÐs¼Ôö×?\<ìWDË?0Ï~ê
°j?up\€C?v¹)'ÿ³]?[¥Ü2ÇX¿?ïï¥?rº:?PýöØ:q?!ÿE"?ŸcW§¾à?^"2²± ?O&û?﷏š¬?€äáȲ¸Ü?Dl—¹€?U.Ü,ØMy?€ÕY+G?î•Û-<–?ïsPŒ+ê6?Œù:ïCÃ?d:^»Ä13?vOØãäõ?ŽERrþ?ŠËC€ujÂ?瑱閩r?rl#
7c´?;‰cŸ%ø?*¨fÐ*Õþ?"{:ˆçð•?r1æâ䚁AGN4FGL J2009.9+3544¿æTáž'W?õÀ—Ì:À9«ð©JèÀ;8&1Âð«@ 'ã'ØD@‰éÍ³}?ÑBDþ·«}?ºëÖÂæ˜?ëȆ·>Æ@	eˆšî®?ïÜyGêz]?䪯k"¿æäMÝX‹1¿Ûì{ÿ)ì8¿çgš®lu¿ãÙÎ"7bmAGNbcuB2 2008+35?ìáêñ{ÿ?°×ù'ô?DG–#Þy?>¥!"Lµ?¸È8Œúª?°ÉÅ?~‰ã?åËlú̆Î?Ë©reß>?|ÌwVÚ÷?'ìú—á|?Óõõ›ß*Y?ʒ}—@µ
?éLJ¾zÏ?¬Å͗1'F?$P$,Eˆ?‰¯6cê5=?ɶœßŸ7h?¬
dY«Hí?èã³Eèª? ï:ÈÄM¤?…ÝÑO$?jٌD7»?Ëõ2e? ¡F^¤Ÿ3?çú7ÃT—Ì?Àoº7žÒ¾?X%و8õr?Rel¯ki?ÏæÕ??¹‡?ÀcÅz>?à;™ï;?ÍñL¸.I?‹ºž¾—?¨d¢ë±?ßµ3P?Í;~ÅFµ?ä	ÉNàZ?µ"ñ›ªE?—}£±ÚßÞ?E'Ç¢M?ÖX2)n?µEvpŽw@?â	Kïö%?°!*ÛS€ä?'ä|I…8?ÿÍÛH›?Úä© äëÁ?¯Ë	þ+u—AGN4FGL J2010.0+0726?Êß9¦®šÀ+}|o½'=À:"ãY×À;Ô¨ÒÁ'@7ŽÆÞ@M˜¤§Ö?ѓ Ì"Â?Ì5¾=gêu?ùZÔG'‡@Ë-´™$T¿ïÿH è?ïòøp¶L¿æðf…p¿é$©'¬¿ïÿëþ@bF?ä"Ä?µwœAGNfsrqTXS 2007+073?îϞo±¯?¤±'Ø,¿`?ˆü^31È´?¡Iòë¯
ü?™ŽðFåÈ?•'Ô'¬cÃ?ï,_Ð'Ó·?œ'äšu–î?Ì®²qj?ˆÓ+×6lª?'€ÚyìQ¹?•?ž)]?êÏPgWl?§»òâo¨-?¡C2-õg¾?"Yñ(šÕŽ?Àqóf®N¡?¥&n­?ì²4'ñÉJ?"ùŠ`?"Ëå°Ä:?vuIï¿kg?µ­¨wákž?' øÞx›È?îàU¬Û?¤h‰ßÅÖl?Š•è¢$ß\?‡…r.ˆ¹?§ì"t¯¯z?¢?î<#)?íœyFN)??²÷,8@ƒì?—¥Ç´»Ý1?£q.é½íc?ªe‡¿¯z?­찒»v?è7à±Ü¥?¯°r'~é?¬~ª¾ùÞ?ŸøuÈ9?ÈûÍCö?«+—·°õ›?ç"SŽiÝ?«"h³Í?¥Q›žÄ‹<?'V6yf?ÌZJÞ9u†?¨W'­c½úAGN4FGL J2010.0+7229?¾',Zz@4*Öý¨6ëÀ8Ö§i¦À;пB Ž€@œÞ¬ôd@•ƒb¯É?¥f¦R9³«?º‡[>7Å@Ñ2^!‡@Oø0Ó²o¿Ã¶¨@οâƾ?ì)4¿ã<î
ö¿ä'õÉEY¿ç£S¿šµ¿ìcÝ ÁAGNbll3FGL J2010.3+72284C +72.28?ïé¥1õ'á?_2I—c_|?Pi¢I)?Iz˜²°|Ö?\¯1éT•u?U?%ƒÁñË?'iä?…nÀ\cô•?lņš«íÐ?tÍ
&É?ƒ&úLû?~ôHîܙ*?ï«ÂR9L—?'m±#C?m4P@ƒÖ?{
AµG™?{"®¿]Zô?y0ȗÚaì?ïEo%Û9€?n›%"îŠ?}붳5?ZúfW\¼#?®[9åéy?g"Çèpô?ïʦÐA?s˜ø™¸-?[-¾!?U!¡­êª?sáQÏåŠÑ?pEïm£?îå%QÚN|?£.SXª'?:í™M}?‰žv²•½7?›–
W¿&? ÎBÙŠ?ïea¤ñ͞?'§ß0cÜ?xz0ø
]:?ƒ3k¢xÝ?Šj~<àŸ×?‰LiI¡‡ð?î³>u?‹2lŽÉ†ò?"êˆe÷?w«ùJ0´)?¤bVÐ/þ?" MŠCݝAGN4FGL J2011.6-1546¿Ûî²PÛËÔÀ8°0ã͚RÀ:vJßø#À;Ю2­Ò@ûÒBØl¾@–ž<–‰?΅ ¨×z%?Õkã=|D@²fŸqIï@é^‹P«"?ìÓÀ§$œ—¿æ"Ÿè¿é­Á±ç¿íŒQGpÅ¿ïÿñò÷¿àšÓá*ÕAGNfsrqPKS 2008-159?ï£õ\7?'þvhi,^?s{
±`"þ?t9!.¯Þ?{zº3£?yˆËºÙÓ?îuoòðç£?¢¢`0¥
ý?"5x·ë¡÷?•ˆOõT¹?žˆäÏÿ°?—çßatÆ?íPz­Vv? Ä*jKs?–'ß,P?Ž\‡†Êµ?¯öA¢M!?š'Ì–}!Â?ì;ü-ô–&?Œ‹è$Bà?¡¡ˆ?BúÀ?y5}LžI›?µOZpKÝó?‡¬HŠí¶%?ïA*g\°…?"Cшj¿‰?‰¤yîÃ?‰B'p-³?†aYï÷?†.VE*-Z?êñ™Ÿ<µ'?¼
·gy¥¢?±µÂ¿v°³?³|A‹Ñßû?¶½pGí}½?°>Ka1±?ëOÝ1˜¡?©›híþkm?£WË#Aˆ?—dàéà?»Õ1ñÐÎu?¥@Áðek?å%J‰³iò?£þ"ñÄFú?¹0"1®#?˜êßñèq5?ÎݽÇ i?¢·¯;8ݏAGN4FGL J2012.0+4629?éÅ.Ê\žÖ@sò«´NÀ7ùvjNRÀ;+ü™C3@щ³¢?þÌÀmBùz?¡ð}^®Ø?¹DŸÂ'­C@±þë-@°fŒQ®?î~Ó-A¿ÙI‰`çK~¿Ý%=ð%—¿ÝæúÀ¥÷÷¿å2Hø"¿â!Ý Y§AGNbll3FGL J2012.0+46297C 2010+4619?ï­¼òlÍ?ŸÀÌÅ+s?XÐœ+?R•fe?À.':Y?Ÿ¸Fszø¤?ï4%@×5±? "Âo;?Qa…«e?Y¾\t±å?˜eG—8‰?ŸÃ*WY'Ÿ?ï}äºÝÀ?"}Z‹Ì-i?}A!àô?"8Tî?˜ps#›ã?
=~bG?ï¤zÄÓj\?gáÆ»?QžÍ±áPs?;z¸³?"­uª.þ?ffFá[ê'?ï‰(âï›P?ž"¸Õ¿?TuÙ菍?P½zÕ¢I?‹'—º?€ÕÕÀ¬z?îGw/XÕ|?°PÛ=ªÉ?g•®™'1?ƒA¯}²?ª;±VÛ¡?°0p÷i!?î¡EUÛºâ?™·6{ÊÎ?~'H°ˆŸ}?'Ú-Þ_œH?¢aŽ°õe?—͆‰† ø?ï,fžM;%?ƒEÜãO?bùþ#ÕôÉ?P^hg?˜ìr¹ÃÌ?'ŽŠû¦¾îAGN4FGL J2012.2-1646?Þ¦çô#0À96½ÂmÎ:À9‹¨"ÉX¤À;DŽŒÂÂ@ê¾¥AÃ@¯ï¤h)µ?¼Ì8A(Ù?Øàc¢¼­ñ@³}pn'@	˜JA¿Ç¡QHòã¿ágºú<q ¿éÖæ+B¤¿ìKâV¡Í¿ïÿs+(x¿ï`,Æ1¨AGNbll3FGL J2012.1-1643PMN J2012-1646?î1ƒÓ:?±'ۑ£»b?­"ƒ7?°öÍïeÍ?lÖ:úÉՍ?m›#'v?îD"²_kÔ?¬Å·'(\í?™vª£¤Ì?¢ˆ‡JýùA?ø¿n¶?›½Ì«t}?éP
'‡i§?²k«$Õy#?ÃÐÒ8?°W€÷4 ?®ß>Bʙ±? q¶x7ú6?í©ošÂŽ…?'3¹L½? E*+¢›?'Ó]IT°?¥IÁ)«u?‰‰kì;?íNnÅR?²°3Õx?¶@Þä[Ǘ?²Y¤ëØâ?xjꁁŒ?tã(Š`?ëM¡}?¿Æ2ᡪ?±¢³C®?· >º…?³õ))/~g?®Ù•FÉt?èT4œÈE?³F•Pß?Ɣ7vò®?±*mG'È?°5ñZt
?ŸKÂ6 ïÝ?ç"RŠ'hô?«× g^Ì?Àˆbz¨]?¤¬F6É`?Á&S[œ³Õ?¤®µ{ö'.AGN4FGL J2013.0-3717¿åÇF½Ý#À?‹UX!)EÀ:…Þ\AIvÀ<OÄøÂôÝ@'T-©±@ØIёX?Å6>5è?·æ4|ßN°?ï/_¿_@%;Qå¥â?ï÷5¡L–\¿à—¿9fS¿åÜ=ƒMÕ¿çUr¼Å¿è
g'E?$¿ïüÁr%·AGNbcuAT20G J201248-371941?ïŸNší?v'5•4±?M}Ž[öUã?CÛá|N?†T€'´¯?umvÝKYù?ïŠr;Ô?"ëih³Ï?`ïÊ(†Êž?dó?,­‰?‰'~t$?%?'†¡uØ3?ïW¢‹Æƒ?y+‡=Ë?iîk9Ö+Ã?a¿&ùÃk?'ÍñÍÓ¬?uÛã-Eå;?ï
9¶aw?q@Ì"– ?t4jåxT?R³ˆ4ļ3?™«É"òi?næñ"üX?îõ«ÕJ8¢?"]êºö?a³…0?T¦ƒeb§?Ÿ$¬!À?'É¢ãÔ­?¨¬‡?žŒ3Ch#?tµ±…z$?}™¿eýQ!?¢ÿ?FÚˆ?š7Ü5ž¾?îhkŠùª?•¤¢U7¼p?€¡¾,Q;å?w¦ËҘ?¥W9ºÆ@ë?'$
€Ÿh4?íeAi=?Œá76#ݾ?‰F TG¼?pçƲ[N\?±­ «Žg ?‰²÷ð":vAGN4FGL J2014.3-0047¿ÙíXð©mDÀ2¿õÆÁÀ9ñÎWçG¢À<l­¨DW@ >eû²hs?ÿ\ÝP¨?¹›ý¢È?™µ ü"?ãcÓCßRá@
±ÇP·?ﶿ¹Sž¿á¦Ç…ò¿à7@=ݱ!¿Ú1Å{`¿æmP›#•¿Ô'xŸ£ô¼AGNbll3FGL J2014.3-0047PMN J2014-0047?ïõØvp—?>ûel.µ??$
#FŽ\?R×Be¿?QÎQsC{K?<Ó´?]ö?ïÜP+;ï?p­+æ›|‰?<õmnÃÀ»?FÄÐ"}¢?p"ªEÔ?n@ýôW?ï»rûRϹ?pm®¿¨šf?V¥12¯Ú?fÐ|Du+?|"©7ó=?f£¢`*u¿?ïMm3è˜c?nÒ½Ãj±x?a‹¹ßÃñ?@"ákŽÈ?" âA¶Ö,?m®&Oˆö?ïîôÄB?Lé¡{u
¯?5|ì#Y?$L‡üu"í?\Ók˜œ+?J)¤òÙ?ï£:æõ‡?"•_1Ş%?H1ì#Ã7?U+5Re/1?…»Òuû|/?ƒwGÃä?ï‰Q\©_?y@åà-?btCŸ7Š?g/¡Ä‡/?‰©˜8?u®¶Kh?îL&8Ù?‰¡­É®3?v¾#×jž{?^­š÷•?«³y$ë-?ˆév¤îAGN4FGL J2014.5+0648?͘xUëÞ¥À.ï»À:
†¢F†À<MÝÙd‹@!/òù²3?üæÑáÃô?¼"À^ÕMz?¥~ü¤¿?íÀSí"?üÑPÒÖQ0?äÔÀ¡›EÁ?|jâ"pv¿ÕN\¤›«B¿Û'oü'7P¿Ø<EÀÿd$¿Ü‡5^0·ÙAGNbll3FGL J2014.5+0648NVSS J201431+064849?ï~1÷?‰5.D:ß?Rn$Ҝ–?GuƒÞqü?Ž.q•_p?€Ë_á#]^?ï'öpéj?‹óR"7å&?`Ÿ,¤\ñ?c¥aƒ:£
?‡Z mDèB?‰INü³?ï(/ìñt?…Ãr£&?l™Ò¸èO?cƒ.±¸Ü?—jŸ²Âd?"wú¿ü":?ì"ji;"?Œ.j‰|9?)ÇØ#öˆ?hzŽÞÌöá?¸7s¹g©?‹L¸1¸žg?î¹£7°¤?ší73Y?j®ù‰—·?]ú¥TK"?¢ºÜê
?š$ÈÆ´®?îäúYç–Á?¡•R)—?sÀñïëd?}U´&⑶?ž}D‡ú? 'ñþ¸ìÁ?î"	àÝ®?šHÀ=¼?{"ü΂•?u²U1E¬a?ª{Yëf'?˜~Q¼ ²F?çՒ	=§'?¡¦ÝCÐTæ?žÃù>­˜?"™u¹ªX?ÌÑ8·Œ?¢@iÌ~F£AGN4FGL J2015.0+1621?æS¿J¶»À$L'ÿK¥À:{gkÀ<™%ÖS^@7Ã¥†·À@!Ì{n5h?·?äq"&Á¿˜Ýèº$dÊ?ã K.Ò{b@5O&óû?ïÿíöé	¿ænyÖ]¿åjŸb0w¿ågÕÒ/]¿Þڌ}ý0Š7{í6OAGNbcu3FGL J2014.9+16234C +16.67?íÇmoo#¤?®j'¯$"þ?d[
á²{?W"Œþ;ì?±!¼+Á",?®+aîâ•D?ëµÌ!?·0.CzÍ'?kÀ	ä¾Ä?vÈîÉßK?À¼ì§Uu?¶£Irݱ?íºŠB—¢?š•§$OHE?|Œ˜[]?uÓy?°bæqg
 ?™[¹V{Ì?îïw6Ò"?s)Ò3V€(?o'("¡Ä?PG{AÀ´;?ž/[$ë|?rCÄ>ü?ëXÓßó?´4yO|^?vö?•tÏh?jÜî*²›?ÁåÂ!øù?³Ëä8ôõ'?çb€â?ÆWr,Ã,?tû*૵?ƒ4yi+r_?ÐéÏú 9~?ÆÍS§¿D?ë#O&"?¨á&撩b?-¯ðÛæ>?ˆAOÿÓ?ÁèiF¦¿?§°~ûm%?ìÌ9',t?OÉ;Ô´¦?‡nEÊwÎ?r§³ø'?¶²•#ä?ŽxÔ´¬AGN4FGL J2015.2-0137¿ìWQ
õÈ*À3T?Ä;-ÓÀ9+O&®ÀrÀ;¹Z%æC–@ۙC]x@™ä"rÁ?­'w-|?¹;#ÿŒ@}ÔÇm{@êñ#?ïý´'l¤¿Ù妢ì~™¿ãgwÞ]îÉ¿ä§''kþ¿ãå{ð;fÞ¿ìY!¼AGNbll3FGL J2015.2-0138PKS 2012-017?îDÛBËŠ?¢}ÂÜbÉ?ræAc/ÎÇ?qó%Î/K?©Uƒ¨â$?¡uQ­©?íŒX+1©?±zX»^äˆ?¤N¹¼ֈ?ªè~¤¸Á?¢ðàŀ'Ü?œfç)j=©?ì¾ÓÒûe?¢~bf+?"ÐÌ>e?Ž	
oäw5?´Õ.WAµv? ¬vrÑmk?é|—Ÿæ²?"@š¨L
?«d»;`ñ`?ƒ¼ÄÃö-Ô?Ã4r²hâ0?¨V¥òü?ëKö`øpó?µæzÐ2?Ž&wuóÆ8?‡óá$!ç>?Àí¿QQ?´¥{®"ߺ?éJAb¤?ÅÃèY'Ü?¿GFŒ< ?ºÈëc2L?¸VgjÈJÝ?²#'KZÈ?è±\ÒF'è?±Zâô¡?£hŽè`ˆ?•š¿‰mQ'?È`hÑáž?¯T–ZIør?â	wuWoþ?¥.åRÐ2?¾r`&¨­«?›%ÍÞ´o£?ÔPy
"Ú?¢˜"¿rÐAGN4FGL J2015.3-1432¿ëèü¦.RyÀ9›Ø8;À;`þ{›ÑÀ<º­æX@!NoæÂÂ2?ÿÌbäѦP?Ë+¿ 'Å濖HáxÞì"?ÐÀ¢\‹Ç@
°s3©OÅ¿ïà¿]x?ïúkHMw¿åL8½¶¯¿ïÿþó…õ?ïÿü¿ÙŸC¿ïÿý`éNäAGNbll3FGL J2015.3-1431NVSS J201525-143202?ïíÒ¨Pc?.àì?%¶Î¡à_ï?Bœ}VÑ%‡?a"Àv:4}?€(¨"Bÿë?ï˶TÍ?‡¾ºÎ8*ë?Hüõâ'Z%?c>ÜòÒJ†?w_•Ý¼z?"ÿõê?íb\vM*?¤$¶b;Ú?"Ùa–ÚÚ?–µQú×I?¯m‡Í&Tw?¡3Í½Ën?ïáá¸R}?]ۊg½øu>÷×Â_ÞÜ>útB»c'?mñm?]ÄÒO""?ïígÅi´­?c³Õü"š:?,,Ѕ(O0?6ž³í÷Ñ?`Õm½@:t?bY7RÌ[†?ö³ë?•X§×Œþ²?K|fü|kè?b¤^|ÀŸ?Œ`ûÿ{†ð?"ý/f,?ëþ`¿À?©.÷'` ‡?'I¾Nª"?"¹ñ*4"?»º_3AK?¨Ájz'?ï|`ˆÖÔ?…˜:˜ Ú?šËú?!Ç\ùÑ\w?dÙæ"2Í?…"Â:ÍhAGN4FGL J2015.4+6556?áaù}Á-@0¤_¿ƒ8.À;tÿ†]À<%ü·v#s@t±ë@ËLÂPr?ßF¿¢AÞÈ?ái¥`!Rá@kÕÓ܌@ˀ"düY¿ïöµ™ª?ïd!È`¿æò
¿ ¼¹¿ê_ ®
ë¿è:´|lb¿ïþ†ܕ˜AGNfsrqS4 2015+65?ïxP>õ
?"(WQÎé?‹<'eDhÀ?'´Fí'Ë?j½xfY(x?o´"¥}Ð?ìló0
å?¼~&ó$«?¯®zð>Êt?¶
Þ	Èò?©¥ÛäpA?¨LBê.‰5?íïÃàüõ?œB‡SY?•Ùóòmª¯?þŒû`?¦Ç÷ãÂV?–¹o¡V?ëLj"`‰F?¡¯YN­n?°ì·ï]*?"juú°‡?´¯óvH?xYFT?îÕá"ð?¡:Ãä/Ç? ro©É!#? »Ëµ°Ž?q{ñIx(å?qwGG,Þ\?çkê‰Ì#?ÈÅ#EDÐ?Ń¹¬ù6§?ėa¶_3?¹™8XöŒ?³	«		'?ìwáO)¢ª?¤Ú¬¥G}?¡bËÙ5?—­¥åä=?³rD|"? *3jcí?ã;du܌?·](*ß?÷ç"
›õ?µ{JØåa?Ï[§LñÚ?¸ô}¸4ãAGN4FGL J2015.5+3710?륛N¿D"?óFç_ö	ÝÀ7OE0‹¹À9¼°´hQù@ 5ä¾[@¤H)í?¦~qcß<U?ÆÀtå/D;@"vtÑc5@TÊH8(¿Ü	"(™&¿Þß9K{(•¿áˆ\ZséÝ¿æj>B(¿ë'"ÂÀ'¿ížè]RlAGNFSRQ3FGL J2015.6+3709MG2 J201534+3710?àV&ٙÊþ?ÏĞRïnÁ?Îÿæy5ï?Ë
iµ{L}?ϧ~>œ?ËgÂBR?¸]Q.R?ÆĞޅ?Óâ
Å÷'?Ð)÷ 5?ãN×(›U?Ñ/Z"
žØ?ÓЖH´ØB?´!QºUþo?я{"‹P?´.Øé¢?ڟî"À
n?·—ÞάöÄ?±KÒ4)x*?—Îujü}^?¼-®6‰ª?¥ŸdÎz¯?êPâ#Ý;?¨"–3(c†?ÌQ
B½Ù"?ÃM ôÏË?ß[õuH½š?ËÝø']Uà?Ò{…jk6b?ÇÁF¼|óq?µ`h8û("?ÃLKL¸?Ø4û=D&?Óe±\{Mv?á9uZRºk?Òß"&'Þ6?ÒAi•^»?³ê[ŸHe?Ó|òVð?·¢þúö?ÚBñ¤U?¸8°ö'}É?=ÕBÁ?|/~rÆ?ÅÔ襁?³Ä®ÕœÓV?ê=qKò?´ùÐàMIXED4FGL J2016.3-2331?éIˆ½±ÚaÀ<†·þ®ûÀ:Ò<!~|À<°¹ßŠ>³@˜¥àyÒÕ?ÿï¤h)µ?ÉÎu™_7?àc·_}>@N1ÿVŒÕ?û[(g¨/ß¿éò^VÍl/¿Ëº!úP¾‰¿Ð2!zÎþ*¿àY	†'¿îZµUů¿âþ@Bæ/AGNbcu1RXS J201604.8-233049?ç¦_ðÖl^?¿#›Ìµáà?ÄÑm§,ª?¸cŠ.þ¬T?¹*%WP>?¬(lMä—ø?çµ£´êFÊ?÷/.Ÿ?Ä×CU6µ–?¾GmŽ	(Ú?¸¤[«>¶?­ZÒ"eõA?â9gê¦Z?µCZ£E²?Ñ×'r¯?²ƒˆ(v?Ãl%‹2:?ª?ãÑy?éÙ¢í\?š}·Ìñ›õ?ºHkz]¥^?•ïOèýXQ?¶êƒÉ9¤?',Sö?å*ùæû!?À£'†¤?˗ërîù·?¼
ÁÛ=d ?¿x`ê3‡?®‹–['—>?à®DZ'µ¹?ÈÆÙ3ɗI?ÓuöÍã^p?È ÝOü‰?Æ[ùòl;?µ¼Þ©ÂQa?Ûä©ç‰Un?¸¶z§-Yi?Øküî'»[?¹ìˆ\?‹?Ç^²TÞo?±m]•KE?ã7Y<K#¯?«¾~Oר?ɨoÀ';¯?ªU¿Ú]õx?Éz+NQ5–?¢0m[þ!'AGN4FGL J2016.3-0903¿ï`2j`qÀ6÷ƒ8.D·À96œò®3À;ÃÖPM'@²ÐG«<?ý¸¸É	É­?®ØŸ¾Ì®ð?µ«½ž¹þ@ŸIc÷ ]@+3¥Cò?ïó?Ýæzž¿ÚS°àˆ¿ÚsŸŸB%¿àáö?6÷Ž¿ÝåÌ¿çÀÞLQkAGNbll3FGL J2016.4-0905PMN J2016-0903?ïñÆlò'Ð?QÐ\æÓ¼?%×*­éôi?Í»…É]?Y¸A+Ä«ø?P™=lj¶?ï×J¦[7Î?sî桍ðu?Aÿ§üÚú?IìíWë?r·Ù!!>?qÉïòUK?ï'_5&:?~ؕ'Ðñ£?`=EYs2U?ZSMºA?‡Xá\j¨Ú?}Z÷Žì"N?kS­?}À'™ß©b?gõèV˜?Fë%"…m?£"ä]Á?|Íéé!q?ïà+^±?c9ð0?6ó£8"?&#Ž}v&?m\]3ñÏ?b',êÀê?æ½8Û?…lY¹g'Ë?UÅX?ÙH)?e¶ˆŒ¸H?‡›M.0?ƒUY£][\?ï_‰pŠ4T?†ŽÞQDñ@?jŠ5>Îaj?oa¾¨q¸?½‹Ih@?"¨‹ßM¬&?íšTKþþ?—Ýý¹¾?xfs
fpÚ?bz—%ld?µŒÆ.Ýiü?—N.·"–ƒAGN4FGL J2017.5-4113?Ã4֎'À@µA•Ì…À:'~Ù#óÀ<yÌí€@ Á-Ý2ö?þ¡™'ƒÒˆ?Á†~Ëb?¶æMý8ûI?ö¹Ö ‹%c@•èO	R?ïŒo_3l>?²Xúm¿Ú|²ÙÀ3¿àÎ1†ŠÉ¿ßÂLì¿äڅ‡"ݘAGNbcu3FGL J2017.6-4110SUMSS J201729-411516?ïæ{~?dß?S>§¼=Ò?42²ëȉ?!§"¢›‡?fþ+—›9?R+¼Í@ß?ïȎfà‰Ã?q?PS#Æ]?Dj'˜ù'.?IBYï¤ã¸?y+zV,7d?o6QX1ÏA?朗;g›V?nþfí[ÍÛ?TzÃý½$?<¯µ'uÛ?'Ì´7BÍ?m€&,Ö?ï_ðoX[?hž"'pd?d'6íM.?D8²ZzÛ?'q«:—/Ñ?gփÀûn‡?ïÕyé_n?b'3ŒP±?D`pÀÄn?5Þ@Çoªö?r¶üøÙÜ?`Œ¾ß`7¢?ïX9Á±ƒ?‹ ¡#:g'?V;r…x6]?^«Ôl™ÕU?"•¦sû-?ŠBšæsô?ïn(xUbn?ÖþQ›¨c?_ \Ry'?aÚTóíæ?Hë-s?}Ñ"2Jñ?îXœBì9?…*ÃÿÇí?wƒÈKŠ'?`'×ËÚe?§½/…Zœ?""aSÿqëAGN4FGL J2017.5-3753¿î?ï,¯F»À@E*"8…À;ñ¤óiðÀ<Ö)làÔ@VæÌzm?ý
v
HX?Ôá5"Ç$—?ыt¨H‰?ûLv›gÏó@E¼uÎ.¿Ú?%ðz|?ïïUÑ{¿ÖÝ~`X/l¿áвÀ12þ¿ßݜÞr'˜¿ïÿý¡UûŠAGNbllPKS 2014-380?ïì<)ã"?]DrÒêx?3†OPzØ?&Äl¿m\?aSYa?\H†™D/?ïÏ$Û¬Ž"?s$JÙè?D=??OÅúK¼;7?uìÊo*ªV?p÷"uãän?ïë²
p?2.ã,´Ž?f%îÔÕ?l…Úlj?Š{—ïÙí?|
ŸXYå"?ïošÂ
?htæ"?TFw…âöa?9PmL6†?È@D?Z?gxMiß%?ïÏíFâE?lCq—cˆ·?KM~$I¶Ó?AŒ¤¶té&?tŸÆý0þ?jsqÔ"Ã?ïW€¾ñÖ?•$Ø Bá?XNê'C½?mv*²èÁf?"ŠùtžÙ?"Š"þéœÀ?ï/ÑÔÉpw?ˆmzŸþÂ?lW¬/
"
?ql¿?–zÏÚf¬?…€6šf‹4?î¸Ã:VO?'ågQ'Æ?]*3Ež?Ríæ?£ŠzÁâïì?'5'7=l'AGN4FGL J2018.5+3852?ÖÎNãÏ?ú¬løQÀ9zeEÔöÀ;Œ 4Rî@ ²þ¤‹:0?ý5¤ãc?À"úˆÇº>?Ò2¿-{@
}ܤ±$Ñ@󟳏%¿è.Ê榓¿éàz~¡Eµ¿½yG'R¿Îk~¾¡æÅ¿ãÊ^'Ӄ ¿ë–BAn	sAGNbcu3FGL J2018.5+3851TXS 2016+386?å–xŒ{u?À˜DF£Ié?œÉ^G!ìS?'ÀŠaQÛh?Óy—¬Q?¿Äî­®_¶?ÔR7<N²7?ÍüÙor~£? 0Ìô·bÝ?£2讬Z¤?äÓג~Ç?ͳï4š€8?å<zl'µ'?±ærêà†?¸ª€h×?£Ó¬Á½Å¶?ÏA6K8?°‡Ü²ç×?äÝ¢}Ìg*?¢ª ƒíÃ?˜ÆÝ_ò"?€
[óÓ?Ôk.–Z8Ê?¢cèæ;'Y?ØygÁ@Ë?Â=oŠ…D?®}Bú:>? Y~i?áÚDK"W?ÂòljG­¥?È[Øгƒ?Å8PSƒï?¡mEï­æ?«Ý¦‹Zìª?èÒ5lüá?Æ(©9?ÜL"Zjè?µW+'®W'?Á†¸yâ"?ª8½zŽ*i?ÚðÛÉ®¤?µ½oæn"Ä?Øîlqd¾"?ªçD¤ å?ª0^&A¿?•Ï­²Qà?áåÃåXÅû?¬"<œ/ÏeMIXED4FGL J2021.9+0629?é¥ÃOÝÌÀ0Çñ"<:CÀ9Ô¦ló"À<›ûs©E@hþŸ'¼³?ÿ8B·4µ?ÁzØù«Ó?ÃW"üÑÍ=@uîþOý@s''dç?ïùd:<;ð¿ÜÔ¬ÀþZ¿Ú­.â@§e¿Ý•+uϐ¿ç6‡æ鮅¿æ䡟øXlAGNbll3FGL J2021.9+0630PMN J2021+0628?ïÀ+û&?oõ¸,B…a?[˓«ß½x?UFïc‰Áý?x÷—®äU¿?iìÿï¥D?°Ø®
?…!WP]­?cs:ÙÌ?fKS2¨ƒø?ƒsÐÅÊ`÷?'Iä˜ ß?ïTÊäóà?…˜0Ö*e?p[¸šá!S?s|º¾¿Ý=?'OÎøµ®¯?'JÌ1:ma?í»×ÒÂã?~ÜVÁyzÊ?Ž¹:b–<?cÄH`U?¬"4>›Ó"?{åë"+sû?ïv"s9*?'d¾Ÿþ,ª?wÔÄ%P÷à?q›zrŠ?†üÕ·†?xƁ‡"­}?îá—fñ?ž6\ñ85'?~¸©)Y–?†HS‹*\?œGo'nŽ?˜€®ñ]?îs>g³‡E?—÷Yä†?ˆeqöqÉ·?‹4Ë?­4Ä?¢²½sK@?'…™œõ?êªâß³¯D?•ù)QQ7? ‹**ªƒ?€>‰qéq?Á1©ùÁ«?"¨3j"ðAGN4FGL J2022.0-7224¿ÎëÀ|v7À@H6âëÀ;_~À<½~«Ê@!"˜`©G?ù§»/ìVÖ?Íҟ_+^©?ÊâÙih7?þǧÓï?ûðSå…U¿è"'|É?ïèw'î\j¿â
Lõ|¿Ä›Ï¿Ez³¿åY"‰ê¿ÄãA-qÓAGNbcu3FGL J2022.2-72201RXS J202204.8-722538?ïÖ¶È 1?d»Ë²@f?A9Z:ó??0,µ¶Ôœf?r'Ô³,‡?c""_áý?ï]´óVJ?Ž@†u(	Ú?o´]™¨ýú?r?E—d7D?RÕé?Äó?‡q§ÕJˆ?ïf@õ¤Ã€?}€|åHa ?güÃêõƒ?bÅ@ _{¦?8HÒÉêY?yÍÎñ˜ö?îŸ8À'?…W.¨"J?‹×LûO?p\î"žï§?¨ÄX‹¼Ÿ?ƒÛ<O/I?ï°âƒöÍ°?uN-­à¿ó?Ra¢ÎËÑ?BY<ƒï?s²ÀŒ@£?tC~Ç+W?íÿÍS–'8?¨½ÇdAÃÑ?ƒ'L"{֔?	o\Ř?«"—Á"Û?¥´‰ÄkRª?ïsŠç$<?†lU£&‰w?qG؜
Ð?qD<'s‡?™ŸÍ3{·Ä?ƒõ`2Óc€?ëoJ†ó
	?œ¶gdŒ?™~Ct@f?‡ßæÞZŽ£?¾&í}W«?›PØoD.AGN4FGL J2022.3-4513¿ïéñJÛpÀA;—ædNÀ9•s³VBÀ<þ+êi–@±ß*óH·@+sKQ7*?°šï¯û°»?¹ü¨ ‰Ò@	1eәo¨@§@,ÀÓ?ïö+ÖGŸÒ¿ÔçÃK•U¿áÃ1­÷õp¿ãmOŽ³ŒŠ¿çätôž¢î¿×|0}d/AGNbll3FGL J2022.2-4515PMN J2022-4513?ïéfýKUû?UüÞ³4S?3È" Õ?*¥nKq'?d »»<?TB×fëÞÁ?ïÖ>3Ô?r˶kDC<?E^ÑZ!§¬?P9'ªI`?r50¢Ðž?o'½ê¬:Â?ïN×Áþ\?ÝðEÖW?m'ÃÝs?vÑ,ېÂ?'se'"·Ý?ŠÝþDáRã?ɾ-*?bôÈÿå?Y \Fú?=;äܼ¢q?†ñi'ªaõ?a¨Öû[Iã?ïÎKÉ=\h?o¬em$î?EÐåKë?<ò£V©³4?v7A\¯?mw³fF?ïuDoñŠ?Šú6&'"	?X13¶C:?fØí-ž«s?¨½›Mñ?ˆxNø	Q?îÁ µRîÌ?—¥‡£Ü!?tAÓ:¡Oê?vÅîÃ3õ:?¡]ºF<™F?•óû"HlŒ?îþë7|Õ?€éëԛ?l4Çm?UܑxÔKH?œœô+̽?Bð22"VAGN4FGL J2022.5+7612¿éC¡Êˆ@5#1;â.^À8éÃ5tVÀ<²<'Î@ÇäX¯™‹@íòœj.r?¤Ò' ½ÿn?¡ñrsï¢?ùÿ¢È"§@oÃgp~?ïÏ"‡"‰¿àâ¢Â7G•¿ä»dàTi¿âA3¦ö¿åÍ·þßn¿åòGAGNbll3FGL J2022.5+7612S5 2023+760?ïëé"¡s5?W'‰œžI=?4eÝ(¾-¶?((vç¨Ñ?aŠ!ÄÝRt?UTë1H?ïÌÀt=®P?w	Z4êny?Quæ8›?]¶£hðòU?uBLCæ	æ?ruÝËj(?ﰉÇX]~?|[pÁžo?aŒ³Cj?qy1»(%‰?~õ
Ä?8?t"€2T?ïÎ@üä0…?YÑt?q?a­•±ûã­?FFò%$?p¶²Ús?SÚÌïyKy?ïÕ>ŠC)9?k6«ìåƒ?CUžîX?9ÝÈ~=ð?röæJá?hù°OÿtÒ?ïz½."?Ž€gÌn¸?c&¹}9¼?tã7büÔ?Œ‡E–ŽØ?‰®HÖį?ï|¾'Åc?Ï7†T?cþ^$ƒ"
?gŒu;7ÛÜ?‹ÐÇІ@?€ys¨©
?ïv†±¬Ø2?xç¹ùå^?z/ÂÞ´ó<?e{w~Ámõ?…Fr/fWÊ?rö±O~AGN4FGL J2023.2+3153¿äþŸvcšÀÀ½gý?[`À9¡ §?tŠÀ;oÆÐ3‰š@!]´8×7	@qú[{PÙ?¾lðï÷ä?¤R×¾Bph?ênwÂYV^@lF__áè?Ö£e_Ö)m?ï±ß`£-í¿Ù¢'ÌM¡¿âç!A™'"¿Û؜cÎ[˜¿á‹ºžLèAGNbcu3FGL J2023.2+31544C +31.56?é…)8?³Hø̗ä1?kɏÅ÷n?ZíÌuŠŸ?É|Ãa¶uÀ?³4ƒNme"?ã­¼T¬?ÇÌ£x%ç¬?vJ¢ 2ô?~E…ƒ–?ØL*¶?LJ½Ù¿Ïc?éfw~^!?¬žE­?‹óªõ&u?'Ù[®V?Ȧƒpý?«¼ã÷eñ"?èßtî?¡˜—n¤«ú?"6õQԝ¡?uIüZ|uä?ÍÅÚ%Œ?¡_öRÄ0?álÕöc–u?¿°ˆ@y?ƒÞ´}	
ð?rˆ 0[Aa?܇^o2N?¿¡Ç‡àÖç?ÖÀ"Ìdê?ÆïJ/ùíÂ?w¯çµð‹?‡by 4?äpV­òÓ-?ÆÎ,j¹~´?ÞÃé—fl#?ºXUŠ(Àò?ž(}L?Hyr[?ß[cç8¼h?¹ÌMq´—?à\ÑTpðƒ?¬aûay†n?£ù3ÌÏëª?K#øC‡?ÜÇ6݄!…?­)šàÄåóMIXED4FGL J2023.4+4127¿çò}ú	y"@Õü¦¯+ÒÀ8ÿÊñ*z'À:ÕKoj'@ wýFKê@Œ~»ÇÁË?Áõ…Rº·÷?Ä·Xtû@B"~ea@wóòUk¿ïÿôa¼2¡?ïÿ
ÂPÇï¿×£aÔÜ;¿â(orŒ¿èќªÆÈ¿Ý#®ÆQˆ‰AGNbcu3FGL J2023.5+4126SSTSL2 J202336.19+412527.0?ÄPøgS™?¹
½-_™?¶$sDÙ?¶#$B"?è'3|‰¶?Á5ö'¹êX?×¢àÓr‹ì?Ç©òÚJT?±Ê ¹Í°f?°Úù­?áõK~ƒ"ž?Æã8a_/?Ü«C•%?·LˆÌpE2?¸Ùٝè<?¦úUç«.ô?ÝF)M?µô·¸Œ¦?Øq<5îØ?¦ºÍ®ºŒ/?«	ˆý°"ˆ?†Fc-)Œ?âM.ќÜ?¦<Q÷»Û/?»XÞúˆ)?³Kàï$­¸?Á-‡Í"Gö?»
L'™ñ?èI'-Ií½?Á:"¬ÖZ?Í!ÔÜø?Ãå:TÃ.q?¼–\¡6?À¶1]y?å$Ðô›?Æ=p¹P™ ?Ðꢒ³î§?±ÚIŸ¾Á?Âiۈ&€?¬&,Ð?âðg?Ãÿ
?³î~Œó¤ð?Ç~>>ª	Ô?¢p;µå^ý?±àÁ€¦I$?"¬xö4Dî?çäX?î=Ç?¥]ƒÉ
»êOTHER4FGL J2023.6-1139?×vSʾÛÀ9­Ð¦v ïÀ9Y´Ñ-"žÀ;õSì^ó@w#Ñ@yî?ÿc<Ù¥"?¯·Úø3­×?À­aw"6-@ã9:´0õ@
w헝•þ?ïÿ¦n£¿½eøØCx{¿â<XuâÛ¿à¹_²˜¿åë'H'@	¿í'¦ïnAGNfsrq3FGL J2023.6-1139PMN J2023-1140?ïå|«™˜º?^ƴϾæN?CW'Œþ{Õ?;Qd¨?¬»?e­tP²s?[¾눆?ï'Å©å8¡?ˆ •ÍŒYM?iZgð¡2«?sŒ­%|6=?"÷ûšW¿?'A§ˆ?ïwÒܨ¯Y?‡×…F¹=?säM¹?|Oˆ>€€Ý?ˆA=¹©A?'‡sx.ý$?îmƒÝ‰w?z¶Ë6RU?Š»áßÁb?e~"Ú¹Q?¢y$J‹_1?v-+IJ?猪ûÀ¼Y?zÎËöj?aª?Œ»m]?^ij?¢võ?o±&ÌU?võƒÀµV?îÂ4è? Ð¸¯RvA?'m¯"¨?ŠÑÝ!c?ž´H ÊÈ?š¶DäÐ=‰?îþqDƒÆ?˜jÙáµ?" *ØEÑÆ?‰l¯"&:³?•áÈI"ÐZ?'D'1;D?ì‹ç菩‰?'AYN–_)?œsáVÐ#ø?	è@ò?´ƒÈdܺ?"0@\AGN4FGL J2023.6-0123?É]ȒÖ[íÀ5þ÷ÂDÀ:[§ŠóäÀ<U›ÍP€K@ÁË[ˆ'ß@Íp`»?ÂeãØ×ó?ם 6×,¢@ÏÄ~I±û@ù(uj?ïöŸ>I;Þ¿ÓG>'òŽ¿Þh3Æ)ñ¿â¡ÎAÒ¿î@;#Â|è¿ÕS"g*±"AGNbcuPMN J2023-0123?àd
m0ï?Á*°üü?Òj¦7ÈÕX?ÀÜ*g [?ɚ‰Û­Ý–?µŒlÒ&®	?ìru3Äå?±Üa,DÔ?¯• ¯•1ë?¬È°V¡+Ç?©I·ù¾ãÏ?¢J¤sOI?Þ!$šÄ?¶Ó4ÁŽçJ?Ö¾Ûôn7§?´­0e:¦Ì?Æ?ÿáïk*?­ ú,žœø?ë%¼K0')?UØ_ä'n?¯øt¯)ö?"ïilÆ å?¶ÕãP5¼>?…+ý×(<×?×ó'6Y6?¿£%š)ž?ÔÙ·cP?ÂnqD2Va?Óï¤Cy|?¾s´"ÊÂ?æòµZ%¢?Ã`Sz®û^?Åuª&.½Ù?ÁsûØБ?½ƒþ
Ú=?²
£1Sý1?Ó_Üßiˆ?·»Åž/Uƒ?ޞ¨j^?ºóånÈúI?̉õm5?²øïjË??äºbX~‹?¢Ý_ÚºË?Áª®è"ÛG?ñÖbþé?ËkdzL6ÿ?š/Ú	â‡MIXED4FGL J2023.8-4828?åã?!uhÀAz»˜Çâ'À;L-ê
ËÀ<°ìˆ3@@CÁNêHß?ÿû©Y*=Á?ÑØ
¢gÉ?±ÉòQì†Ñ?Úµò€:¢é?ÿ·	Øi
?ê0‰jwm¿ï5§¡ïÿW?ÝÊ3)ø÷οÜĄ¿Aô¿ïþÍ?äF'?ïõ@‰]tAGNbllPMN J2023-4826?ïÅvÊ6Åd?m ©\Êü&?V:)9é¿z?Q#â'ñ±¡?w¶‰Z8?iíýÖ¸?ïY'BC?9Á¿íß?\åÿɅb?b09ڝj?…&þ»j q?|.bQK|¡?ï7C·æ?ŠI|_qáŒ?w–Hª1x
?~fAØ.?"6ê|>?ƒÂ©®rÃ9?ïcÃÑGþ?u¢*ÐÏ?XÇuæZ>D?Jd‰ñç?'ûyv€¾?sÓoìàˆ'?ï—O17ýÀ?ëE긨?hmEû?oc-Ð1
?"òª ·E?zÿWñ$J?ïZ»é®?—qÑì€Î?døØXnž?pC½P)¤?œÕ£ÿÜÁ"?•ˆu&jq?p`˜Ð?'Ÿ"&à`ö?{Û,Ùû?€e§;ÓÅ?¡¥m–¿J?b€+H(?î^Á•G?'©56ü=?e–®¿Ä?bËԌW9i?¨ÅÒ݈ó?'VÝ8œAGN4FGL J2024.4-0847¿áŽUÌBíÀ8¥"¦óõ0À9Ë,´"ðãÀ<#:Š?‰ƒ@ £Y5ü?ÿ!{zÊ¡y?¹×Ó2Ó?ªñÆ+rõk?ñˆڀ·@ùyŠ˜?íbfâ(r¿Ùuã'¥¿âg…_ÐË	¿Ü%l 9±R¿Ü
EbàŸè¿è©rÀü¨AGNbll3FGL J2024.4-08481RXS J202428.9-084810?ïÑÝêùªô?`ñ)Ý?Gg‡—¿j(?4"Œ—ÄßK?t$œ×:?]ãFÞL+F?ïºåÕÃ|¨?wøÈî6Ð?Q¨Ê*°S­?RÝi܋?~"⢳Þé?uP"Lr?ïoz<9Ê°?vƒIC;y?dބïaKó?]KfŒM??Žé϶÷?s<R8€}Õ?î'5T'÷?yiƒè‡‡?xzûFy`e?V÷h&¼?£ÍOe¯6ƒ?wy‰ÔX?ï"éVù¿}?x—O?`ØBõ铼?Pn¥Þ'\?†Ï™Œ¬ÁØ?vã3^B?ï,T$?¥?•Á¼Ö,?c½òRd9?q–6%<Â?—ý¿–ªè&?"÷RX3ë?î˦Ž´?ŒX= o?ué¥}+f?qW»Ï‹°X? ˆuU¨º/?‡ªkNÀŸ?ìNÎÉkO?"ºý5ƒ?Ž/,‰
ì?rÂ!\¢ìt?¹Ã¤"<HŽ?"i°WR¨AGN4FGL J2024.6-3252¿ï™=´À@rö@c^À9[ù‹q¸ªÀ<YhQ"2@'ÝžVAÖ@хÞz?²#Š•š±?Ã}ƒa@êÿÓ>×@¸	™¿Ø¢PA¶Ù›¿ß	Û !³"¿çqž]£Ÿ,¿æªõwÖ¿é¼]°	s¿ïÿ³©æ÷AGNfsrq3FGL J2024.4-3254PKS 2021-330?ïæWҜ<?[ãÂù,7?Jšé퉿 ?An*6./?crËîcG?Wd®kSY?ïÖ³íû'?t
ÙÉ?Cº¿®†æk?MÇQ8º·û?r.±+¤#+?q¼Ç²¸ÏÂ?ïš^ÝÓQÄ?zç/ÿ>?gùµœÝ+w?m‰¬çǪ?ƒiÛ""lA?vÙó%¤óÌ?ïǧ1e[W?U§ÑȎ"x?U)—Tx-à?7ÆU62‰Ï?vâ‹rß?S`ÛÙK^?ïÀ'Fõ:ˆ?tµÂïƒ?aþ–"JË?\'ÜAüþ?v¿'<^CB?oa.ð¶:?ïvÖQ.?'A#Ѓ?`Õå­ÔÅ?€˜Òÿ&ËK?ŽD G?‹€»X.Šð?ïH‹ñ:j?‰·Ö·Ý?tÄËà·e?w5ÎÖ(Ìk?'ΛŠÞ¶q?…þðvÐ4ï?ïm8TÛ#¨?v6­t?m)4nÖÿ)?Xg-3[vo?g¶\A?sAÉUI_§AGN4FGL J2024.7-2328?Á'¨MðŒÀ>Rk?éúÛÀ:¿ìMøÀ<€¾‰¬½@o¯YIre?ÿ3-Ú-Þ`?ÉõDæf?ʬ¬è*÷@&ûëýê@ÓÊJ¼?ëM¾,0
?ï]ËB83¿â›6A°y…¿ÜÊ®DK‰k¿å5¯¿ ¿S¿ïÿý¡UûŠAGNbcu3FGL J2024.8-2331NVSS J202442-232826?ïÄ?J¡AŒ?ˆÎ.õ×u,?Vâðôš×?["ø>¦h?x'Ó_äCB?…ª]݇®?ï©?á0Jå?€ÅœÃR?YÑÔ$ ?^"̗uƒ?'r3%?|$Á#K­?ïx'X1ÅJ?|€Ê'}ã?e›}B¢œ?b·Uƒ w?Œ"ÃÇÆñ?yšXò7§û?î»Õê5q?|¬QLæÇý?‡Ò­ƒÓ¬?hÆ[0?œüÙ[°½¾?x]ÿcô®?è¬t?~íkáw?j'Î'+š?`­úÞ²Å;?†yµ×Œ&?xèێð?îÙè"W‡•?ÿRªªž?uddV3?‡&nŸ]|?ŸiöªÔ?˜´/Ôkî?ïœTE?ŠCÏ~?rÅ­8§Ð5?v?՞ӣT?™‹*–dX?†€(elí?ìýÊQGp?•	¡ïrvç?—ø@[eš?gO¥Â5?²)"ö]?'z¥ÎÎ]AGN4FGL J2024.8-6459¿ßLòšo`ÀA'žÓ•>À:ˆ¨½ùË3À<†\S½í6@%ÄRTá"@(\ÅÓ´?¼øӐá9@?£cV9?äÄ°¾Ï3/@ÅÛAÖ?ïý@h¿Ûšðü××m¿é6ù5¿ã‡!A™'"¿ãmÝô<}_¿éMOõ^fAGNbcuPMN J2024-6458?ïë9µ`ýú?fdfȓ,š?6IP›%ç?HŸÓ4v?aý ‹˜í?c½±Y‡cj?ïæÅÓ©0?h^kЕÓ?,C¡èXHÙ?:¥ËV*.'?guòš™£E?f©©Qà'?!ÅÄè?}t7­Ã¬?^	p©¤ÁM?h'þ±'S!?ƒ^Ʌ`Ͼ?y²>—›Á?ïîô4ÎF}?<_¨0{ª?0k‡ÅŁ£?‹|>e?]ü´"^Ì?;ÂôÍ|q?ïÕ¼?¿L?wÕzó÷–?Eîu¤ú€?RÛ0}_G?rd/½¥m?t×ÿÁ¹ù?ï°pázÀ?ƒdÿ;e'û?Añ B­«>?V¯õF­ª?'ÛÉÈÁ{?',ƒæ±Ô¿?ïf£›ƒ²/?…iÄҝë:?h0¤ŸÉiÚ?p —"ȲÖ?%xǺÒ?ƒj÷‡÷y?ïÊÏÈsÅ?_À\ë­&ƒ?JžDï¶@J?6ÔWŒ^õm?wDS~›©!?^5ªôçôAGN4FGL J2025.2+0317¿ïúýÏÏ
ÀÀ3`4óþÀ9:yÂc½?À<®Bž
B@gÑØÐ;A@†ÛPô?®h¼ày/Ÿ?³‹ÉLd²‡@çÖs>»ý@«é¯¼'¿ÜFï}¦ÉÙ¿ßða<æ¿ã«DAM}6¿ß¥Iû÷‡¶¿çnÅ°xÙ¿èç(bõ˜žAGNfsrqPKS 2022+031?ïõ¿åÖ?V/ç£6¬2?(Ï·å²?3*DœgL‰?Räˆú"Æ"?RADÌ?ïì)¾Œº…?hQ¦U\°]?3^øŒö6Ü?C\>qÊÃ#?ajbp¡Ìn?e=£«Á'g?ï`Iƒ¬?Œ‹ñÌqÄO?ZÏÄÉR)Ó?bÃqgú?'Pº{¾Â?‹êoè'?ïÓP¾¼Ñ?T*/• 8‡?HrK±vB?*ÐìtÍý?sIPÍ>4?RâK	24?ïê¬E1§1?sb\RӗÛ?=sqϏ?HLâÒÍ?a³Ly§u?p¬ðfïs!?ïÆ4öå?ƒ–DIô"?OTù†&^?eɧºÔ]?xóìýÀôË?€‰Ýń?îð߰̈|?"Õ'e3z?i´öIüV?rPJ,3c©?ž­k$ꄾ?"C"R¨†?ïŠ}–ûüÞ?s›xdhP÷?`Ôô³q?Lƒ,—þÿ?‰+™Ëh¸?qÉÄrä€AGN4FGL J2025.3-2231¿êBŒÜ5º;À>"ÓÍ$áÀ:‹Ú¨W¢À<nU•]ʶ@ '6Ö*ïm?ýégØVmË?À¦´_B°ª?±Ìö%‹«?óá3ÁÎl	?ù»fØ&G?ï÷ڂû¿ÜªWA…[t¿Ý¯ïüý—¿ÑÙ÷¢äF¿èíòKâV¢¿|>ûq-AGNbcuNVSS J202515-223016?ïl$pÒY?ˆ5BÙ£³?_u_àÐ?[2Uô›vR?"&¦îýà?†Ö}ö\'?ï8•%t6?"YâF8?zˆ9¹£éî?z2å#;‰?—6ÞçÁ¿?€gÒÚâ?ï&t—ñ<²?ŠWɶ/?t=›"fê¸?z@;ì?–"÷?…׬NÒöÝ?ìRìª\F?'nßì«ä?–€ßA!;?uÉ"©9S?·ä~ù%†?GIAq?îÑÕÜt?—j7 8Ü?tŽôJ¥J¿?m1Ñ扣? \?–Ï×ó?•c¢R*
R?íGwÉmÐF?³jÇ^5ÛÓ?Œ¬@Nõg"?'ôqÙ˜^?².¹¬jžÞ?²=ºóñ?î>՚Éø?—šLL'ي?ÐÍÞÕÄ?¦ÒmÇÂð?§Ê² ')?•¨×<Kçˆ?æ¦=`8X?¥tS¡Ù'P?ª¾dÔ?'È™*â@?ÎÇ)æ?¥ykÞÔîAGN4FGL J2025.3+3341¿ä•ÔZµ®"ÀR

ù¾À8A=e¼{À:™-BŠ¿@‡/›#1ˆ@Ò±-4±?²jî «†?ÆÖhA‡ß³@s ÔƖ@ÉÃØÝQ?ïÎxžwNì¿å«ã‰o€¿çý"såªê¿ç8?!(οï-ád´`¿Æƒ~_pAGNbll3FGL J2025.2+3340B2 2023+33?²Ϝ?²*Ÿ,G?šHöfë?±Af«õUœ?'As™¨þ©?ú'šá\?äe¨3mô-?Í`•H¢?ŸiÄS?¥ÀT"Ôܵ?Õ>—ÂKa?ËP1úÙó?ãúÈ/Œ¾?´ˆ°RU¨Í?¾·
æÑ
'?§ŠŽC7(?Ð^:öÿƒâ?²Ùv'#Eº?æ<L'"ß?©T/ŸX_
?£Žï$C3å?†ÚÄ×ìØ´?ш…þÆ?§¹Q#kçp?íPlL"h?¨†™Úٖ9?¢%c2ùø?žvå/³?¨ØÆ:˜t"?žïHZáC?Ýg!DÑÉ¿?Ñ6"w4s?¯ïh»Ò¿Û?¼pœ1Œ?ޚñ£EêÆ?Ð{`B#Õ·?ã¹Ì+\?³‰Ï–™X?À‡ÑÕ(§?©¨3B[?ÐH}öX"õ?±nÊp`—?Ö:ô¿ãŽ?±š˜e–?».~`¶¬­?£ÜÛˉ?á|ï9‰8£?²»rU¶ MIXED4FGL J2025.6-0735?æ\©»ÈÀ8cY§TmÀ7"§&J¥À;;A¼bò>@t‹gÒ¢$@ƒÅ_AË?Žµë`ðR?¸ÝÊ @&sü"$íö@ Bî «†¿Ð7X[á¨&¿à9RÂÀp¿ä¸;æ`Ê¿åýÉÄڐ¿è½jęød¿ëS/uKAGNfsrq3FGL J2025.6-0736PKS 2023-07?ïBüCÝÐU?™u¹¡"[?q‡––±?"ðÉ[r$\?"\՜hѲ?"£5À÷ƒ?ï¦Ó£5?ŽÛ'œ×?X"–L½ä?qጛ†
3?ƒ:a&\r?Œ½ÜN?ï«ɇaÍ?…‡Jϖ‡•?z2*Úª'?'uXTÔel?pJðkCå?sµ
ál#?ïæˆ`>âœ?XÀÛyÑ8Õ?Gì
†by?@O'eãŸM?c$®n?S5¹RûH?ï6¢CêÄ?™*ÊDawÍ?nwdXβ?q$™G{H?•jȔ¼Œ¤?•ö§ý÷?ï6K4Ë}†?¢Þ}P-?s¬ú!¬;Ÿ?"¬·má?"KZÝ¡OS?Ùk/'®ˆ?ï¨YÝA?‡TÓ/×!ÿ?um鰼ڔ?Æp ú&?v'éJ¥l?|éܼQÕ?ï¿mœCJ¶?s)	>ë?[F8W
,?S¶ÿ3Ÿ
?yw£ßE…Ó?p»E»sý‰AGN4FGL J2026.0-2845¿Ö7ùÁw"À@"ƒ‡ß]À:˜i6$;À<Míض@HLó"Ìß@dqcðja?͘+ˆy?ŜÆʪ2Ä?ö–•ˆ'á@	Þ'h#ֿ湓¿ºëy¿âÇ`Ƥj¿èýب£!Ù¿è"u'À²¿è¼ÕÞÄF¿ïÿ½ÅGóAGNfsrq1FGL J2025.9-2852PMN J2025-2845?ï˜	'µÀ[?°±¹U̐<?|ÕÞ?Ö¥?°¦#g1?w&f;1P"?~­¸EÌ&?ï¹|A*Rö?'òŒJ3Ôf?Pe£ÅWè"?Y£áM†r?(v˜m¯?(+îrpT?ï‰Á)'°?€¸š
‹â?emì˜ø:‹?prˆâªî?ˆ`TŒEßb?}ëvæND?ïª[¤5~?`Pû;'N?PÄZ_?1v?((p3?ƒP‹¹×.ª?^>å12S?ïgUÀ'"?–yiK¾²g?i¿ÓI#™'?p€Ôѕ?ºÅît,ò?"¥»5ךŠ?ïêùøBá?¢Àãç6)?aª®kð?qMPC??šÁ+cCç?¢8áòòÓ?ï)È9ÙÚ@?Š<›n¯?pã:ÖL?q°±Úç?–Ž0ùªÍà?‡
"?Bʦ?ï{…1'¯?~·ÝŒðŒB?cVwãÞ?QŃ?U¤y?›%À\e¬c?|ѵùyc¦AGN4FGL J2026.1+7645¿ïü¸Tg,×@59>ê ›À;
æ_E	õÀ<«­	¸æf@"Š[Ö?'<?ø›%:L,(?ǝ¤ÖŽ—ˆ?ÆWe—‰t@‡ÿÞr¿@T=ïϱ¿ïëUN.K¿ï×ßàzԈ?ïå³vQì?Âv'^¿à´€€G¿¾³ÌÓ¯ëAGNbcu3FGL J2026.3+76442MASS J20263126+7644487?ì^*O+Y?Ò·¨£LÌ?o폃¡ÐÂ?'› þvJ?¾½¢3,cq?ѝaäQ¶?ïŠ&ÅÀÂ?‹H1&u?cxܣŨ?jTejºt`?ˆ˜œ%{j?‡E²²\m›?îITv"Ÿ?  ‡rEZ?iÍåÖ§û?ucUp?­ýÞë?Ÿ¸ˆêp?î8#>ߏ?‰¿Ïÿú½?l_
"×ê?\íùŠ"?ª·Ýlü.o?‰n3íËӆ?î$ò"ä£?ÀDÓúò?d~#0ێâ?sèÏ0Ç?¬w®§çÛ?ÀY.'m?îÜIê&F]? S¨›*˜y?uòô.³˜.?BK¯ô´?žú§û*Z?œŒ{
þ¯Ë?íZûN?~?£)Ã-ú€?rãâ˹<Ò?zøÜ%sW?³ùç`ڇâ?¢"£??ë
)K̪?§ x­$ø?úWÒ«ZK?}¤—b&w£?·¶'ö?§Ì%AGN4FGL J2026.6+3449?×͍™ÂE¿ÿu
xŽ‡À9¢ZÐ0.œÀ;?Ö§A"	@ s¹£¥60@CÂÍoŠ?Â8Éu)wÉ?£ùÉÁ:ف?âUKÚt?ý3ßJӸϿîÓAáKßÒ?îj»_¼þù¿è`¼mÙø.¿Þû]Ay¿ã–,A§j=¿ç¡®pÁ3<AGNbcuNVSS J202638+345022?äqÁõiŠC?»æbÏFéb?pDS1Vj?`×E	D;?ÖÛl=á?»á2Vᰁ?áÉø††cÔ?Éa£
~?ƒÑáG9?‰… _ÓNJ?ÛÍç¹.­?ÈÝÒ艅"?⻈N:?³ÿBÐ(?–2â"N?ˆä¦'=æ?Ù'Ü5~¿?³¥ém0Hâ?äí^"hÊ?¡ŽÕU¾j¸? -HäO"K?~ccº(6?Ô™àˆ¸Ã? ËQô$»²?Úâ1°Hª
?¿:Øûє?ƒ­ß1`m§?v[Ó¬>?â@/«i"?¿y¦'O,ì?Ñ®ÆQ¯?Å­î‹õ}V?A-`¥ $? á8ÏáF…?æ«òg/x?łЫv?Ô6¹B´ä?´ÏxT£»ô?£žðj'™@?"Ï߀øp¼?䪴X%Ÿ¼?´©È»ÆL?ڒA³ÿv?ª6œdÉ/?­.ƒÄAÏ2?'('1v–?àã×"ï¡Â?ªhW´9ZMIXED4FGL J2029.1-1839?æ®Od¨\fÀ=£·•-#OÀ:°dPâp£À<kَ|/&@ˆ>	P
Ú@ÙaÃiv¼?Íe˜¶×í?Ó@ª; g@EQÄ?ÿc‡ÁÕÍÒ?ïßÓ™hF¿Õú,@ûÆ¿äTž›·¿åÿ`h¤
¿åU'ÿùJ¿ïÿqšw+AGNbcu1FGL J2029.0-1840NVSS J202900-183709?îýU·}Á]?Šj60'ä?o–2cÙÞù?aƒÁ©¢¸?œb'½EVˆ?I
˜¢R?îà!Lo´?•{çÞÊE÷?ƒµü…i¼?€®õS°'?š!NúÑý??eSχ}'?îz$°}O¦?"éǀóà?‡¢weq†Æ?'™}L)w?¢uΣò?'8'ŸèNo?챓²"ª[?‰ìþæ ??Ê¤¦ð?y/â!eô?³âC¥é?‡ô¦W.?í̙¦5?¡úrÁK`è?ƒ¶³ž'Õ?wô#Ǿ½?®HÃ?ÁÅ? sJ´yÝ?ìL/}"v?³'®Õ?Ÿõ©4Î0(?¢W>pJ?µ¡Çzž?¬=IYâµÇ?í.ÜŸBÑ?¡ /:A±?•^¤EÝ?Œ(ì¯G?±B‡zbe´?œPž%?çÖÑ>\Ã6? ËM™+ƒ¾?®²Ëýk'y?"A7F¬üg?ÈøV'Ì? 0ªn5°AGN4FGL J2029.5+4925?†øMÿÉ@ª@]wúã`À9õ6À;jÍë°½£@´Øö¦ºê@×R9ˆ·Ê?¶ÌMöØäÞ?ÓA­§m˜@ÙgÊêt~@ó,ª-®?è$ÁUuR¿É/¥ßøù|¿áÓ+UïÞ¿èì›Sþ¿ëF–½FG¿ïø3þ_AAGNbll3FGL J2029.4+4923MG4 J202932+4925?çë å7?Á%hÇaw?ÂT䢛9Ç?À¬ÎÙÜ´?»ù5îEåµ?­"<Õ½D?î'w±:±?ªAê PË?q±`g'ž?{Àç~n'?«Rkì9?©

[×?âjÌ.tæ?³FF¾pâ˜?ÏÍ+w'(ä?°)"ÿ…'?Ɗ•X"?­Wã(ÊG¹?íäß5¸§/?ˆºÃ.jÞ?ˆÞ·sÝÔ?l½cÕ
?«z^ÊHŠŸ?…mæYÞ7?çg6Æ÷±ä?¹ö)H"Ù?Â
4þ¼D?µ—ãË#ÑØ?ÀXïæ|,?®zø`ý°j?ëï8ZÂ?½í\¨nì?ˆYƕ² §?"zþLAd3?½|¥hÀïÛ?¼ÐšÑkÜ·?á6áÛt&æ?³Éiñ§Ö?Ñ·hUÚ¹?²ÕÀ
}•?ǵ§æ¨.÷?­‡H9ð^?êWŽ¼ñ¸j?¢å¢†¨%N? íÊB_Ê6?†ÜâЌx^?ÂfR|F?¡"uÐAGN4FGL J2030.2-0620?á{sâ-¹À8Ö®::ŽqÀ:GÖ(ôìÀ<%o•º@ǯïœZ"@qƜ1#Ž?º…࿝å.¿¨>,œ§QN?êG±ÚØÿ
@C×n;qñ?æ*K-$ü9¿à
è`ܺ¿é·<­/x"¿ÜÞ>ÄáÆÚ¿êˆe>É…¿Ä5»"ÖCÄAGNfsrq3FGL J2030.2-0622TXS 2027-065?ïä€G/‹Ö?. mÁv?Z`~w?‹Ìè¨)è!?\=`Ê¥M?k2"6dQJ?ïí@w?e÷h'G¹%?,'{þэ?=°ëy€œ?a#ÕèUp?cs‡	ö?ï¡UÈ3‹?šµá–bù?j3ôÍg"s?y#{®ÄÈu?.-_¶!?tØôøY?ïëÌ(¯n?BŒÛ…Î;Ý?+~†ÿ£˜?NØþå7?b{ö…׿ ?AÝn²3—?ïçapC›?`Þzgñr?KË{ÃõW?J="ìÕZâ?a¿Äò%?[A@'f?ïÅ0άù?ÖO®Ç.Ï?@.ZÉÙÚH?Pú™¹Á	?{aÒݤâ«?}Š¶^܄?ïbéŽúYM?…Ä>…b/>?m]ïÀ[ì
?t†÷þ	ù?î ?̯Ø?'ý^SŠ#*?ïÂ
ÀvÁí?b¨kӒ€¢?F|½4m ?3Jê
þÁ†?|)‡ÿŽy)?aìox2"›AGN4FGL J2030.4-0502¿åù*g¡iÀ8Lma,jÂÀ;,,"ÜÁ7À<ƒØÐç
Á@ ZÑÜV,²?ÿ•;fœ?Ñw'w?«)ˆ9ŸÞØ?áj‡þf¢Ì@'šËrړ¿Çӈé:x¿ìxþžÖð<¿áÿ®ÁžñG¿à
ïAkÛ¿Öµ»€Ê¿á·1$e:AGNfsrqTXS 2027-052?ïªF~¾w?Œ…nÓî
Q?1ÐÇæ`\ï?&‡ÚÜÁ?"ßö¥WJ¼?Œp*¼äo?ï±H·}Û?~‡W¯·»µ?SDY­7´Œ?Z3vÏÄU?Eq
T»?z°ç¿>ž?ïYdá3¿©?'["°"´'?Uˆ®B{®*?;F]µ"¢?"zØ÷?'RsósPï?ïd«V8#'?mèƒÍ)?<£N/­&?$NÊ»âŒ?'øø—·ß?mµ˜ð¯?ï-ÈOº}j?˜8s;ÿ²?A""yZq9?3›\EÄu™?™½áãºn?˜"ÜÁ?ï5âàŠnÙ?•õ¦R0?_ù¯jф?kT¬wKÀ?—Dÿ"0Š?"Üö¥36Ö?îoÃ㢰?—Ê;ð=Œ ?\£¶\T¶?LmöшN?¨)R?—¶ª'"žù?îûív»s?a'áM5´?Oý7Lª?Dþ$wO?¯ J¶"4Š?|¥=–AGN4FGL J2030.5-1439?Ün(ýzÀ<o"}cÀ:¶Fà‡•À<yŒ†‹ŸÜ@ çþ¥aùÅ?ý©•?ÇR¡ãj?žŸyzÀ;?Øß#¦@@víb£æ?å•6Þcx¿è»îQ"ñ¿àÍ,¾¤ëݿׄH"S6^¿ÏU-Ä^iB¿ÕC¿ÝÑAGNfsrq3FGL J2030.5-1439NVSS J203028-143918?ïµ[ø?­(ñg–$5?;+ÚÊÞ?*í:™A¤¢?e³×ìD?­*ý™C>‹?ï»ß…Ù.?yu«‰ÎMë?Lxõa¶xé?Wþ3]`¿o?~á*Å?uö IýË+?ïY€Ù>Ü?~ˆÜh?XDºãùâ?@™™éb Ä?"N«MýÚ?}¸^{?wH?ïcD…Àô§?kÚÆË,ÿ?LÙ¦]flÈ?2‹ÐŒ)®w?'°¢¦â[?kª@é#Ïy?ïêr²?œíˆe1
¤?Oƒ6Û¯&?@á³ë–?ž¦˜{Ø?œÏÜ¡¬¹?ïThU»³?1fíYf!?UøXÇ7{³?aoòu5³¬?"o½_îé?ÁjB|å?ûǔ²?"½·%ޛ]?`rÌl?OåpÂzgý?¥ã?Ìeø?"w–ke?î*yP×fŒ?‰Nœ@v?a& òZ"?PÓÂf—»ª?¬GèLÎ?‰'@"	3=AGN4FGL J2030.8-6959¿ÑË2Id‰(À@ç]þ¸Ø#À;¨mqóbÀ<²˜§+R"@WR
é͏@ځNš?̧ jْ®?²ú2¡ì?äyºHeÊ@ßËZ'œ?íqD îÍ~¿ìKIt¾þ¿ÅCŽõü›ò¿ç.ðäJ7¿ÜEva†,Õ¿âg¡yâÅAGNbcuPKS 2024-701?ïÏ$‰JÜ?mbئð{E?6ññp4>(?(ŠÜ¯­ç?vþ݂ßé>?lªÇ©§2?ï¨ðvlC?€à	·,0?Xuf·?_R¦ P2—?'ÃBa-ÕA?z—WÔ4¢?ï['Œ7Žë?~dǧ_Z"?aփ¿[z?`*Sè>Ö?'Rþ?19?|^Ў"ú?'Œ°?`Ù7íî·¯?K>xS¼çÍ?1lâZË(î?‡gÓ§º6?`T»_dY?ï‰EgN~ú?"¯+¬J.?Iw>eïZ°?=,,lH.?Œ2IôØ¿?"Z $m0§?ïÁðƒhÞ?šR';ān?aÐô(KB²?p<»_£'Þ?œM£d9ê?˜|ohøÏÑ?îËììÁ£"?‹ó¡Ë1?l>$Ol?gA
:Æ?¡}OAHÚ?ŠIÏzÊÂ?îÒ¡P$ä?ÛV.¶"ô?\mŸÖJ«?NiÓp}?¡ûXèƒÊk?¤}3ðûAGN4FGL J2030.9-1621¿îÌiÊÀ=0]¥qÀ:®p¦[HüÀ<~b¼ºh@]µ%ç@…	Œ³?ÅÛï?z?£ö AÏ?à_‰gó.`@œ¤MQ¿ì0Ï«¤¿Ú6à;êfç¿åyÄ6%¿×'@~b¿×.ž
œ µ¿ïÿ"Év7AGNbcuNVSS J203048-162224?ï†[ê¡õ?¬ünh"?Js)FŽz?9îk0¸ª?ŒÁÒé^[?¬	€…—J?ïÃ}}Ú r?½NJRîì?C0š
-…?K';<æ¯?{Ý{"ó?€ÉT˜kÅÄ?ïkå´ORy?{Gí·€ò?_åŒo»'÷?I†ð"¢ªo?"ð´mf?z¥ØûÜë5?ï'9ÅëÔq?hºROñÃq?Ph¦Ó+<?5VÿÒx²?dy£ÆHm?hÛ,lµ­?ï.Ø^â?—qF:ã0?]Š»¡~"Þ?QU¸úv?›áÎûÃ^?–†"ÓïÓ?ï$ÙR¹'º?£¨w"h?T"ÈêOØ?`,áÅô?š"©"M²»?¢âÖU¤ó?îçTÂ\ÿ?‹"SÄõ©?hñ¤-€p›?aÞk"?Ÿ÷I©ël?Šhò‡ðš?î–)õÇÂÍ?‡=ø9à?f:¼':w?VÜïW¯Êú?¥=\÷´?†~»xºÇAGN4FGL J2030.9+1935?êW•âbÀ'
"cØ­À9¢^)ÊÀ;î=ÚV"L@å4!Å£?úpŸM7Á?·›þ£´{?Ä,ÞÅÈ¡š@°iS@/ÅÇ
â¿Ù4åOz'—¿ÚF0ÑY#ˆ¿ÖCÆ=çl5¿Ï;>š@¿äŒÄŸâ¿Þ|Û·Ì5AGNbll3FGL J2031.0+1937RX J2030.8+1935?祥o?|ъ¢¶óÏ?oBE@B7¢?g±¤Žj"?|ŽÃˆÈ"?u	nC¢'¢?ï"`±Šjì?¹j÷–?V#XÍ*á?_´Œ±Îš?ˆchu®Y¤?"íþ¸¼¦?ïV"Xž
?‰´îùaD,?v¯éþfì?ï…Ï"W~?4Û'‡?"¨g2A?îù¥óÅ	?"±è­Äm?xÖâZÁ­5?XˆRà4L?«%‰RSÓÊ?'ÜÚñþu?ïçЀ­Ý?•YõDGÛ?ˆæ
áK&G?'SþË<?ïþúGL??yíÐ?î¯ôg–Y?¬Ûœý´ó©?vês 9ˆ?ˆ"â£ïK?¢<ÜC&46?«šÕt_O%?î´ùiÓÈ?–pw¡›˜?ˆªƒ\Å?ˆÁ&KOPú?Ñ%"<¢?ë=Ñç?ëñþóÄ?ƺßm?ˆmhW:?pÂbpL–?¾ßOúFá?œ"uƌ´AGN4FGL J2031.1-2615?Úoh£Wˆ}À@G¦a(9À:‡îúôþDÀ<Â*²[1@ÀJˆdh@&†|†c?ÄZQDÁ%$?χ>.@bϾÔã?ù²jÉ!œˆ¿ïÿ"=ßßy?ïÿþ½à ¿¿Ü‹©_>¿çN(Ÿ~¶¿ãf[)òB¿äGGQÎ(íAGNbcuTXS 2028-264?ïž;!i1G?€6Ð>ûÍ?f8Ͷµ"?`
ÿ+$Œ?'ïi¬zË?{©
hêîU?í¼Õ•À"{?¬wu²}£ì?œ#3Õ!1? ¶'<z?¦!
{Ó´? |ô–œ?í×g×)È? ^кlª?–@Þâ¼H?'…á:síƒ?§nŠ}@]?š"TJI?ì£D-´÷¢?ùC}w1â?¥Z
‰,T?…	eoÒµ?°8ÙL
eL?…C†Õ-:?ï½Àüp:?'Î8¤å'»?~‡2ì•Ú½?tþ±ªì*?–&{#h¹?'¿óÿï?éµTÇÇC:?Á:©…[/?³€jhfŒJ?µÝÂqtÏo?¾ÔïVˤë?´Që˜r…·?ìÃ?e¶æ?£¶šë°? °ÁÖÞûL?–']l5Àÿ?±£ëºË.?žŒ«ÁÝ?èðp§¡³Þ?£7Æ9š?³÷(›ùœï?›×eôûÅ?ÂB©XI?¯¬ä ¼¾AGN4FGL J2031.2-4121¿½øopƒÔ>ÀAÕ¥~ª*À;.¦Üx;À<³JÖ½ç@m·&tU@?e¦MC?ÎÖþÎ?à­]€ä–î@
¼{F@¿òRBm
¿îCšžý0Ã?ïÿÏù§÷*¿Ü/#" ¿æìÎÊÓοîCÐàWÄ¿ïÿ–ƒd£ïAGNbcuSUMSS J203056-411906?ï©8*$õ?‰vx3?xT•Y?€&ç,—á$?rÔ«g89?wÍ×*i?ïÈ9ÙÚ@B?|a•#vp?Pڐïy'?a­º~À™?w¬Ž´#`À?uú`‡=ò5?ëà–æ:?§Oû*o}?°ðϟ¼)?¡m¹0š?°c¨U{?ž·gF~r?ïÏo'³F>?_æˆSVÚN?_#xçÞ?Få*Ò¦7?p"sK?\þ´RŽâ?ïoM,}a?š­Lþ8š?Šn/¤§z?•? ˆRøµ?s}¥ßˆF?yRìàã5?ïK"z#e=? |küFå?lÍ&¼'Ïô?€ÏDÔvár?'óëé€^K?œ‰',zÂ?êz
\Vdˆ?«ßÎÜ?¸å*lFA†?¤æ]E,?³Jj²¾h7? ñŽZÅç?ïdu¤¶œù?cGšÂ½@?wÔ œëM3?eøgg
Çf?ŠøF§?zãËí=ÒAGN4FGL J2031.8+1619¿ï¶¥l`¦À+ÿŠ:›À:ºZ/ ~üÀ<?Ô|ñÃ@ó2Ûõ^¼@P³''d?É1Á¿"?½ä<Uäˆ?õ^yLò÷Ú@&¢¬ì?ïþÔI˜Ð¿å.)ÿ,ñP¿ìgß?–ÀÓD`,;¿í©¿Ãyè¿ïý›l°ÚAGNbcuMG1 J203139+1622?ïY0çî*.?X+"3)Ð?f^dfÀT?qúpCPä?'ls³»?	Ðáè?ï'ÒŒ™Ü?œU´Þ¿?a,÷õçm£?q°'NÜT}?‡@íů'?ŽÔ©È¸Vx?ç?•‹!¾J?'áQ@Eߘ?‡b²ÿP–?¡>zdû U?'è¨?ïÆ7©±â?€gWH/Q?uuOF<	þ?cVÓ\š?—éå4ÃCF?~=­Š:I´?îÃßSj¾Ã?›iþÃf?s[Dlp¶?täusì)=?¡V˜ß|«6?˜úՊ×Ç?î¯o-ס	?®5Ž®Zz?zÌ˸Œ6L?'¨ŠH#ø[?¡¯s¯%ý(?«Óê*?í~G Ùqÿ? ÐÆì~?«@Né`ñ?Œ/mì!?°^ïWCç?œS¢Aó?í? >#|?š²!ªé…è?"ÂѹU(?†£ŸËōT?±DÂHV´V?™½Íè‹AGN4FGL J2032.0+1219?íq2ãAŸÀ/"š8ûÊÀ9ÃÁc>ÓÀ;ä"Àìĺ@)*Û£@ž®"i›?ÀCŸ¼ô<¨?Àìõ·&È?þ]†Þ«òb@Ç
ÈÀx¬¿±	[]ô§Ý¿åcØ·¼šP¿åʆÁ¥§D¿äG-»úír¿æ¬L#Å&¿ðAGNbll3FGL J2031.8+1223PKS 2029+121?ïñæÖÒùÑ?[96·û?4´Ô[霸?5©"µ€Ÿ ?WDÓ?WÆ'ª7?ïåœl\ʆ?k7¥Ç›þ­?76Žÿõx?B¦âBa^?g|Âß!?hé~K_Ò?ï™"É?|£{"À´8?`ІŠZ Ý?\üS¦$,?……[('›Ÿ?z"´×'Ÿ?ï]šô"?jÝLöú…?eÕ]Ú²'?Cç—ÁP$?''^#H?i·,Ô(Ê?ïæFM
Ç5?bŠ
Ò©ð$?J4‰4G¶r?Dù¡N"A§?c,Í²@Ö?^ÍÂA3Ì?ï©tí#Y?†o5©sÁ?Q_ԃ|Û?`)êF(ó?ƒw:vÚ6?"Ö‡«??ïF²¥óÞÎ?ˆ°ö¤Ùàÿ?py;›°¡Ó?tEÀCŒÆ?"\Y¼Ä?"óSRΆ?î;k#é?†ëXrÁï?~ØCêÂi?coˆ…µ?¨nG`…´‡?†¨.̊÷AGN4FGL J2033.7+6308¿ç:ß²,¸@*øœýç!À;CÛ÷âûÀ<—έwœð@!'x´FÄ?ûÚ®‡ggî?Ì£J(î?Û@=²¾@ˑcj2¤@›KutK¿ïþ³™õßì¿í¯>;¤ò?ïÿÿ^ðP`¿§œÅ+	¿ßŽý'¬¿ì9Z'}rAGNbcu3FGL J2033.6+630987GB 203249.5+625814?í5¯ºB\?»®56\w>?y4YÜ"¨?v*¶Fi?µãèe»?»tÔ±áÿ?íëôoJˆ?°`°.‡¯?Šä;ç'e ?V""?ª‡ªÕØ\?¬M…† `?ë¸ô0q•w?«ý-Sl±?>Pš7©Y?ˆÂ9Ocz?¾P"h¾kœ?«/«y¡ôµ?ì`¯òeQ'?™ê‰ìÀ?Œ™'Ks"?z·ñðÞÿô?¹gNJ"7€?˜ZPÛ(¶?ì·Ñù'•?¹ZÏ Lø<?'·ßÓ®I?ƒ¿H²MÓô?·êt=?¸«RE‡?륤óG"p?¿¤|»VF¢?ž!|Ä¥¯?¦Ì˜MØê¬?»Jy5v'?ºÙ^ß% ?éÅÅoÚÑ?°áŒkÙxõ?™O	%½^?"CÀ(Œ'?Å¿
{rÖÑ?°R»Ò%<«?æK—:—Ö?³ßŸ[;?¢Òï'ÔÁS?žiç>+ù?ÑtÝÁ‰?²óÁa[AGN4FGL J2034.6+1154?íS_ތè±À0Œ¬¯öÓ1À9YiÂ;ySÀ;Žpð›@r¨h3@ÔdcP?½-—ÿÜÅ?Á¶—;?þi¾Å£à@k–JYÀf?ä"ÝÛ
¿ÝÆG·J/¿ægfÁ€Š¿èFl*˅¥¿è'áý¶z¿æXøŠ.ÃAGNfsrq3FGL J2034.3+1155TXS 2032+117?ïðIhÉ?P÷LP¶?; £ÂW±‡?:Æ0ÈFø?X…Ô¬ÉXð?IÐçáW
$?ïÝM¶Êµy?pVR×o;m?ADx/¼c?JQÏ(?nqøD¼žà?lÎâÈÐ?ï-š=¿^?´>探—?oªOã¯Ê®?t²±¹èî?–WnFœ«ú?æ¼ÌŸaw?ïå¾5ZU?rmã'xÅ)?qC…ëõ?O¸¥9"-?™'†[Í{á?q£¬ fž?ïËTå_•½?nwÞëÖ¥Û?Zs/¡Õ§?Yà°]nÞ?s¸ÁS"6?hsÞOð‰?ïž>ÉÌÎ?Š˜ho"³7?Zxüó±j?m1÷4±Ù?…!x€$?‡soœ·Ø?î‡X'¤n?™Rïç.ß?ƒªõšŸö¤?…à¯ÀÜÛ?¢Ÿ¹l"i8?–OðE\\v?í_Eˆ¨ä?I2J–Vb?Š!Ç-?nê­©`'?±Á³bDM?l»´yÈAGN4FGL J2034.8-4200?á« Ml3ÀB3´ÃÁ‹PÀ:C¿šµ"ŒÀ<a,"¹º@ W$"2LX?üsAü#Òm?Á¬ÐB£¿?ÁŒ÷Ÿ´:Û@ô즆çæ@db̨å'?ïþ6Ò$$¢¿ä杞6€¿ß¿YFÃ2ð¿ÎxÕäÎv¿â'jeÏg²¿äìf€<¦OAGNbll3FGL J2034.6-42022MASS J20345108-4200386?ïègÛº$?Y#ý'ß¾?4?9,×>?4û0¹Üªf?e=*Ó÷7?V¤-½M?¦š‡ ?vúi-º$3?IµBºD݃?LÝö%J–÷?|÷
¼[5g?tÄhRïM?ï"À­s…?}X¯0¤ù?X>è$|ý?\!†£uÍü?‡ö2Ì°ó'?|"S/¦?ï+1…oQX?p—5
Hº?j|¸—F':?J2[ÿXc?—J8>}Á?pNº‰d~k?ïÔÑ¥=€ƒ?düõÝú,?L:¤õá‰P?C…Y/HÛ?rØ˕¸Œ?crˆ˜h‡?ïIëñÖ«?töà%Ì?]±¹Ìñ?få¯:n?"çf0T"S?Hÿ´ù?ï1j—^½?Š(—|GŸ?a÷"%0n?WÅ*—Z[Š?—"º«ŽÃæ?‰#ÿÝÇü?íϯ±š'š?ˆ¢b®'ˆ?r~/o7?gÈî}Ñf?¯µ'ƒkt?ˆ3egu˂AGN4FGL J2034.9-0450¿ï㷊p[ÞÀ91öº «À:tBúP"–À<N¿ïn¸D@T¢Ëò\S@b¥Z'"?Æ!Ô¦Šî±?Âþl©±?úÆqÔX²I@Mq6Ô¨¿êá:­z÷î?ïö'÷䨌¿äSÓâ?Ð¥¿äÈ'­ÄÊ¿ãÏ >ŽÛû¿ïø²<'ÎAGNbcuNVSS J203508-045029?$a‡?{²$î2‹`?U²	ïdÚ?L³±úý?‰eµ¸õY¨?z9P‰}hF?ï»îk‹œß?xÇÎç«^·?Q¡ý͕'?T)"?ã˜?} J¤p7£?u¡Ñ–Ìñ?ï+¸d­K?†EkS'ö®?lo]¦9h>?mã­^$|ý?–û´œ%?"?ÁRB‡'?îî'$¢n!?tth¥U?{&-ðor?[E'ŽA#œ?›dP N¶?q­j[(ö?îÝ<ÄV†Ÿ?"zv²œœo?u‹uê¿ÞF?p"}Š
ÅC?žõ‰õÛ»‡?'UÞ#¤Ym?ï
ñH"Rê?›šæ|Ÿƒ?h­<,aÍò?q_òá"?›,/h5d	?™‰p߈?îO	g7?–_'Bچy?~‡·@Ҟ?vªY°J‹?§>r'Îç2?"ÖZHŒa?í~Áý÷ù2?¯wE…?ŒmaÛ¦Õ"?u%4LJÌÑ?°|CӍÑ?Œdôú§÷6AGN4FGL J2035.4+1056?ڊQP\ôÀ1>F{åS¬À7²¼MùˆÀ;4Oó]Z@zø?kQ@".:¥î<?—³®e%0?¿¦Û ¢ŒÝ@"'o°'@}4JµZë¿Ë kÅËÑ¥¿â%¦V]Û¿å<Z#bØ¿æ£Pg  ‰¿ê$¯â±;¿èæÖcNƒòAGNfsrq3FGL J2035.3+1055PKS 2032+107?ïœbïŽmÁ?~gEî‹?e\wÆ|Mô?gx~¥¢ë?ƒ&W 9?w®ôÈ0Q?ïß®]9Û³?rìså¹°?C²B˜†5e?UlöV$?keÁHÖ?p¥åp®?ï"d³Êë?Š"Q!Ênè?uŒ±$·Ü±?€ñ"¡#~p?€`¥Šì?'ð¼È %Ð?ïãAÄ?X wAqŽ´?@Ç|p[å0?4EGñ.ÿ?hŒÓÀ¨?UQá]"ß?Ù!Cò?{-}Õøì?nEN3Ç?iºd¸Ð7?"Šö …´?tz‹JÅØ?ï¤5£êš?|µásý?a6
æó?x"Ôø:?'²-K×Ã?ŒÆ]º`+?ïo8Ò%ô~? 9-ŸÖ?€Çc¬LÐ?‡E&׃€?"%"¤Ç¬?‡n¦¯_\:?﮶+ —»?tJkMFÕà?WÛ6Q]±/?NÔ?o¶p?W>H?r &€"dAGN4FGL J2035.9+4901?ӝ¾ÂH@ë@UZ¥À9‹'ªhô¶À;¸‹C•@ Ɋ8þyB?þŒÜò´½â?¼eáÜ(Šc?¼ØüŸ½?þ‰Às"6Œ@­¸ºÇË¿ïòö—¡qÕ?ïýŠuV¿âé>›A:¿ÒXÚaµÒŠ¿ã€¡{k¿Û‹ÃîúAGNbcu3FGL J2035.8+49022MASS J20355146+4901490?î¢iµS›?"¨6óåž?[$'-{À?NcÌqŸâÙ?¥5ã4÷?"#ûèJw?ì¥)UãP?µ€nˆ'?qrˆŒl¼—?xš…ÛTW¤?¹¿P4?´Sr¸—&F?í 37ÿ‡?(»Ó-Ε?öímèL?|¼SZ.?°¿ˆ'j"J?š'4ïw¦è?ìëÖê¡c?‡¦ÄJSR'?'"A2C?n'Ì@—?´¾êkV+?…£‹ýþÑ?í*OÀ˜È?¦l¡;j‡?vdPáË?sìªL&ò?µG<íî›Ú?¥zn+æF?çTŽïéÔ½?ŀ,LÜt?"Ï5}}h½?'0C;To?аhsíô¡?ÄÝ7–ê?ê
ϸu¸û?°¨\r¸'{?"`0€÷k?ˆ¹ÓVñ׳?Åh»Rk)?¯éª?éHW81Zý?ž½	ä™íÞ?¤
ŒRÛ°p?†_¥UÈ0?ÅÛ@
º¡°?)±ŒüézAGN4FGL J2036.4+6553?ï¾¾Qè]«@-—µÐ1\À9ûžs.À<(Ød°ƒÁ@㬁u`?þº}>ïÿØ?¶_adsòì?ÃÅ£e@	Ê*[]@
,™­æƒ?ïþ;¤ñ¼p¿ÌcÂÈ&C¿Öë÷öFC¿Úå»d°¿çÃâB׿äLD琝rAGNbll3FGL J2036.4+655187GB 203539.4+654245?ïáéeÎÄ?n
"²Úò?7y?:'r?3‰¹Œ‡ ?k'r}Ìb?mšEƒ¡n?ïžôs1§?ŒüÀc¢?b,ãí¶‹?jbàg8?ƒ¿Wøq6À?ˆ¸[ÏÕ,ý?ï—7.ùU?}*»Œèò?fíc,?jŸ}–©.H?"±y(B»Ó?zhÛ?îÇ5ðÁm?vvCIE	E?"²«úŸaè?`Ò7m£F?œ¿ëçf?r"q­"9?ïÔYê¾5–?t'=hy
?Iظƒ3ºŽ?B¶ËÝÿD,?r—óŽnùv?sҎûTxi?îôÁƼðê?Ÿ/h)]g&?x¿…°kJ?‡í	e:Š?›7å¹F¡ê?™-Ÿ|Zå?ïaî-ßP!?"0ÍΙ£?s)K:p?vç÷‹=f?ûßá†Ö?U6ה?ìð4+¼Øt?Tc$U?™3G«bÉ?zé×̑‡â?²1Œ¶‰.?Šó‹Òx®AGN4FGL J2036.9-3329¿ïxÁ†-è,ÀAśý÷èÀ:^x]ï"À<H™¤T(@!$/_>)?óŒïœÛmz?Ð.è¶7_?ÏÏ{¨Â×V?û'ÿ·@¨éÜ?Ž¨ºH棹¿è)!ACAH¿äLXÓÖ¬J¿ÃÃ7Îxt¿Ê/ÁŽ«)¿Ú&èa¨¼wAGNbll3FGL J2036.6-33251RXS J203650.9-332817?ïm&g®÷
?‰-ôS%KQ?S8´¢ïŽ°?FŽÝŽa€µ?''§Ä­Ì?ˆQL×x?ï¤Üb
‰?ÔkÿæÖ<?U&r—¹zú?]Ca>'?"U:‡ÎàŠ?~üèîsj?í©µðV-£? "š8Üp?u
fò?wL­
ÜåÞ?±aŸÜm˜y?Ÿ\"v6_…?î
ðOø?‡ŒX—HE?QЮ?@e¿¾¢¿?®Âz÷2 ?‡xƒÑ.¦õ?î$¤PF?££ñ×Pp?kY×m×F?bAü¥?¬qøû±?¢ð=ª°mF?ï¢ÀpY?™8›Z—ƒÈ?`¤Húèºy?l7Z>Ñ~?›w֖
?—¿Ý¢žU4?ë'Ù˜Qö?§7¸k;?‰4ö³k¡?ˆCGyýw.?ÀaO¿õ'®?¦^n¹?ëá2?¢ª#¡è?\ÚM‡}þU?UU#íHÙë?ÃFÇWËv"?¢°E™ÇyÂAGN4FGL J2037.9-0504¿ïéÙÊ®†ÞÀ9ñD»ó¡À:ý]0\¿À<‹;Óåj@ J@–H+?ûGã>(Y»?Ô2本ž"?Ìÿ9[–S¿?ûTâæÅ°?ý?]Rìa?ãc	¼Ad¿ëI‡î'ð¿Ï1~¨&¥¿Ü&š¢þ¿Óôk0Ñ¿ïü>àŸ°AGNbcuPMN J2037-0508?ïW½¤™Z?—#WÓ8'<?VTšˆð:£?`¢XÖ3?"£ÂåÒ´?•]Sd?ïv¹ªR›Ñ?‰'¤ÿ?f½Œ)?jaÙàð¾ï?Œ¢2_ò°–?…¸›¸8ÞF?îó¢|AD?:ãkü|?p¨¶óg°Y?q߈*Ï>?a'´¢Iò?ŽuçãQ?íq¢è×?‡!y5ø•?n^Û1ÞW5?UÏPÅPß?³ø5ØÀP?†™»—4(j?îŸv@+Ǹ?œNÑÙ­Ú?h7™§äé'?_ÓQqöó?¤…"c3)n?šù",³ƒ?î{D#<è`?¥É!cLj?z60½.î"?…	,\Pú?¥÷²9ß±?£S‹æz3R?î\ÊA"Y?˜Væ˜Cç?wÈÊ¿ð[?y­ëŸU?«Áøƒ?—wɰЧT?éRϪÁŠ?¡ÓYì ÷?w•<ˆ^˜C?kÿÇ8tÎÒ?Éø½Òo4?¡v¸qŠ¬£AGN4FGL J2038.7+5117?å"`þú
@ÿA<á1ßÀ9g{o'VÀ;A_ˆü"d@¦ºZ•@Ó}c-Ø?ÀúX R…ß?Ó±Zÿ@¾6`]'@ˆ"ŽJ[¿â°¿?ñ\¤¿Ûò–Šñ`*¿äÀ~«Ê*¿èÝ_ìú•¿î¿ñQçSa¿ïÿW-ä>ÙAGNfsrq3FGL J2038.8+51133C 418?ê™|)'8?µG¤†‰?¨ŠkçW‹?¡Rѝ¼Êé?¾îèÅ?©}?±Œ™ßmA?îNPx›û§?¨ö÷»p?qqõ«à8z?ziÞÅb•4?¨ì¹½€'?¦Ø&dq-e?ç"N¡?°uàW»?µTOٌAÐ?¡]U"ŽÃ?ÈåP'·T?¬'L@Ѻ?íÛ\e9H?Ï*{ýÈ?'rçS¾õ?e¬L©mÎ?µâ!φÜ?d3)yÖC?è;e—gð?¾Äªû|ô®?©'pµ¯*Ï?¡¿8Ìã?ȱÍswO?»?vsµëp?뒌Äù|?ÁËh¯Òý?‡º¸\¯,?"19S Ën?À=ÑBŽ?ÀN'KéÚÇ?äþ§¾Ao?²­Ù‰_?¸³Ðßä©?¥.UïCñÒ?ϫӞß9ó?®¬rî—ÊM?è¯ãMþ̵?¨Oµ?<?˜*––)ي?µ/•Ð||?Ê;ó‡Ãü?§q/2ÁŸýAGN4FGL J2039.0-1046¿çzPœ¶À­À<¼{՝VÀ8¹
…"ÿ×À;°¿òɶ˜@´VØ~ܪ?ÿK Íj~?¦I³RR]E?·Ûþ2¡N@÷•p?-<@ٔ媿1¿Õ§D}"¿×ÖÈ#DӚ¿á8ãv\~¿àÓ> L%È¿ã¾XˆWR¿èM3>ñ­WAGNbll3FGL J2039.0-1047TXS 2036-109?ïàÕ "†F?`X]F§Ž5?GO½|ãì?@V󑐖?iVð–&?[\{.‰%9?ï'qVÚWO?‡©Æ÷ñt¿?c"ëášL8?l1õˆ:F,?†~oF´ÅD?ƒ´dl±o?ï¨s`³?róBztu?e@žB+6Ð?s]*f?€"΀	‡?{ÒéäïM?î…b¤~¾¼?'«ý7Žbµ?|ù[µV?\ËHˆòçÅ?¤&»:Z?2lpÍ­?ïãüFë?Wá#­‡?Y£.'í\?U'vãoO;?‰R›^«?[Gs6üg?R.ms?£ýLCú?|àІàðH?‹JþÊ¡?¡€È‹vK? #Åå¤up?ï.Å®S³?"T0N"r?{ù³‡™Î[?"éOüúâ?"(ÝOï?[¸¨÷‡@?ìژQgs#?™m0pea¼?‹ôH1Š 1?sÂûâï?µ¬´oÜý_?—ú¨fáÂoAGN4FGL J2039.3+2150¿çÍÉ)wÀ'©K{(•JÀ:"Ï$•á~À<CN"¸‰@z…Nˆú@ºòDUšf?Í»Ûۈ|?хRdÑ»Ê@ø¸BÒ¨@'ہÆi?ïÿEÅÜèìêÿ½ºá¿áiž)KS¿ë¶
éh¿ïö¦…:g¿ì8ÄL0ZAGNbcuTXS 2037+216?íÓ½­R¼™?¥Ã"àà?r'¶U q(?jcŒaÃÈ?°9ç2	Ú£?¥­ҌÔ?ëKvZ5¬?¼d¹tøœ×?HKðV?È^2x=Í?Àýž"m–?ºÚc¹7ï†?î‹]äB?™PfT/É?Œtèa>Ô?†vlqW#?§±-?•™ˆ×ÉbÝ?íhðÉ)'?†"éï/hÇ?"'4x,·n?qëÄ\Wn"?¯¯Ù.×oB?ƒ/OÀþ?ê5 ØÁç?¾­ð錡?…2¯D[?'|ÆùCæC?ÅØגMŸñ?¾ÂÍ":Æ?æä"rF?ÊüÖk»?¡%Ç¿æ˜"?¦:Ô>ë?ѱA>lTð?ÉLÎsÚ²?녋°«a¡?§îþÈ>êï? ÛN¨)?'TÐʄßR?»Í4Õägb?¤Ó'Õ-ƒ?èùŠÏ–¡?¢Q«ˆ_%?¦"]§I?Œû%ø"–!?Ƒ=}lšæ?¡3	Ú¯AGN4FGL J2039.5+5218¿Ãà¦Ñîþ.@[]ô§ÝÀ9èê1ÄÀ<Þ7X@!ž†)þ?üÃPíX]?¹&+¸À{[?¨ˆÝ³N÷?ðcª2n?þ!M:ƒ?ït²ÄãÊ?¿ïüáù?ïöóçÃɿ丕k7¿Øædÿ´¿Ô…qÄhzAGNbll3FGL J2039.5+52171ES 2037+521?éŠC÷jt?¼­fƒÜÞ?qžH´õE?`îB0Xº»?ÉJ˜ª†Pç?¼'tŒCð›?å!¨—çW?Æ 'î?õJ?SrÏÉ?_ÛÏÖ?ÔÀ6õ=6ö?Æ=È*¯3½?ìi¦óÛk?£œIþúè?''‹Juhé?}°ÔÚ‰ç?¼Üa]p§?¢ÃޜÆa?é¦dòâ¤ê?¦#:̍‡?ñ¥oÞÜ?"™Jn'!?ÇH7†ÿãû?¥®í¼ý?ã«dS«g'?ÂùLmÒýz?ƒ>@ƒÛó­?rzú?ØET•P?Âôφv¸T?ÚÿŸŠå?ÇálRIà?—®›'q»?¡Ë—`·ÙS?áà«Vãð?ƛY}ê?èn"—¦¶?­—ü¬%?Éi®o?'T'xH9?Ìt²ñü©?¬>O
õŽ?ã5᠐Ñ?¶ñgAà-?m3¥˜?•"3‹äx?×Ãuꬠv?¶íøçi¬MIXED4FGL J2040.0-5737?î‡z‰DHÀB‡DÃ~orÀ:+jî‹cvÀ<K¥"cØ@mdõxµ@ÉÚª"?ºYF¾U?¢Ì~HZaË?è¢FçE?õ´k×êb4?ï˜Úϐ¿áƒ]©~i¿æJÀ¾¡'¿à¶}Õî´~¿éâ…0V	!¿ïôÚgÀºAGNbcu3FGL J2040.0-5734PKS 2036-577?ïU¹Œöjw?‡Äªˆ²?`Úh¢'Ù?X«V‰:X?"-‹¦â¿?†›æPž`?îØ䗼>?˜H²˜Õ5?…˜"9ã?†!àïQX¤?š*íS$÷?'-[ü×·?îÄAvJ'©?'n‰7±#!?‡Ï)x"Gm?ˆ .{kðº?›<x¬9.?‹kÓ×Ô¾?í4ü‡6Á?".÷"ôV?£IΜƒúc?'aÂZµ†?©fpXtä˜?ƒxû¸dƒ?îËКÚ?¢1Ì[å?€	7T‰©?u2À1¶îØ?«lÀ¬.Ñâ?¡c˜¡d#?솳è>?´<dûí›?œ(}³Æ&Ò?¡lìVCÈ?´ÀAQ˜žÔ?­Àt%¡E?íüsjÓ*?™ËÎE΀?'šgWƒô?‹V\i‹?¦ëƞE·?"'÷Õ^ù?é%\ÇðÞ¿?¤9'0I¬?¹Îñ/?›‰)g‹8?½¿K¢ô>ß?œ—úc\"AGN4FGL J2040.1-4621¿ÓñiBþq#ÀBкs-õÀ:¶€À<p.½'¬î@ øŠ/nW¡?ùâؼ²£?Å®_¹Îî:?Á¬;ç%?ýõÇèa}É?þ1ÿ§?êØ+ÛPO¿ï痞—°5?îõ«þO¿Ù˜*™0¾¿à/ ×{|x¿Çyœ#6»ÔAGNbcu2MASS J20400660-4620180?ï©âÛÔý?sýgAÖ*Ä?DÉ,Aˆl)?6Ðdztœ?":è6P\?siöd'?ï'ßbü?‡£!TNç?b™t¸"Ë?dŽ·ÃBÅ?‹têómC?…#{ר"?ï;Š!Mú×?‡¬O…¢Œt?\]t|¸
&?GùЂŽ6 ?–Èä"p"D?‡]hsv?ìóܒf6?"z9ڜb?r!ÄèQ3Œ?b3›™ì(F?·>ÿãè?"'qì¨ö‰?ï5i‰d ?Žj£Å?^³VØÙÔ?Uvüåž?—sÝiÊkk?ŒÛ<k·?H¨²´?¡YLXhW?sàƒ':á2?uZ"Ÿâë?£XkÿÕ%?ž÷+|!çñ?î™\þØ<?'Ø›0ISC?d#IÜÇ?Y‰?nêi?¥*-î(PÒ?'€ç¦TÙo?é!þò'¿?¬ÍC´ó'½?~)g;¨>¤?wÂlë²?Ê®,ÊI ï?¬ÀñZIðAGN4FGL J2040.2-7115¿ìøP@µ&éÀAs–Б}À9èFžÀ<<é•Zo¸@!Ž^I·?úIޚTª?¶UˆÞ
ŒÌ?¬_‡œcoÞ?÷ƒmjW@H­Ù©T?ï§hß½jY¿ÛÄþø*¿Ô;ýÊ
ü¿Ú&æô–?r¿Ô=¡ K¤ï¿Ñ*=áb.AGNbll3FGL J2040.2-7115PKS 2035-714?ïb ÿT–?ˆK‹¥­Qœ?Srà¯.??C<VfÛ?'"²¦`m?‡³'áЧé?ï~ÛCC\Ý?Šb}¡áÿž?d5áˆÐ"v?h~a?m ½?‹;¶Æmež?†–%é
?îþ'A-V?‹Ì´Ü½œ?tœ8Ìw'?vÉ64wô?›
ÐÌVrb?ˆø"S!™?íD*­¹ÈI?‰ƒÓ¬{?vè_g~?añ+mÃZ9?³ç<
"V?ˆ@;J–?îs0`ŸÜ?ŸÄÌ{­Æ-?mÒUGd(ƒ?aï\\Šå?¦ïÚFq¤>?ž'
Œ©y¿?î†ÚðÚ{À?¢÷Ц&?uó-¶¨èQ?~ŽCÅg«È?¤Óë9Ÿ]ÿ?¡lct|PI?í½e"<Þ?Ÿ—[3©æô?~8ùž- ?~á>]׉?°1HB"3?øO3NHÿ?é4¯ˆ|?¢ë Ùk ?'
ËßUÕ8?z¨´Œ]Ÿ¯?Ɉc*5¢?¢Ïeç)‰AGN4FGL J2040.2-2506?äN¨h©žÀA4'¾‹ÁÀ:³íضÀ<i"`šu@qàqo@àú)&j?ÈQe£Gî+?ÂOÒ:Ê×)?ñÝ t-Þ@7 ¼c?y¿æ*#õ¨Ž)¿å4¢žûÙ¿çe-BŠ¿¿ïÿËý™ô2?ïý1¹¶o"AGNfsrqPKS 2037-253?ïuýJ÷}®?Ê¾íH'Ë?m‹Íï-À?bwÑ˱é?‹¹×Û&_?€¸ò\ÎÂ?ïZL{t?‰˜ÁRQMÔ?qA-ÉÄ?r.5­>ò™?f)bþî?ƒt"p¦Z?ï8ØÅî%&?…÷™ðz©?uµÊd®#–?uÈ
w}'?"wt£e?'¥fé-?ï'©Vê·?xWs·6?|à"4sRE?aÇÄÌ?•7¢Na€?r³ï'ÅœÌ?îÒúB¼>?'`4 ­šd?'­·ÏâÆQ?zZT{:?œIÛÍ8?Õ"
¯N?íîã¤û\?¥Û$"gÚå?‡yKiŒ•ã?Ž8Äg?«3ràQ¡Ï?¡®"
"Ü?î¸BN"…?ÊNʺå?}ä›dcƓ?yNÇÉJ? ¿G¯N\?Š~sÖ?íK€ŒWfÄ?"I݃J?",=ýdåË?xqûu϶?°Øì©m?'µv™åDAGN4FGL J2040.5-1705¿ì Áè("À?—‰Åæÿ~À9ÇlÝxì{À<.œ×%@™ø÷øõ@l—E+ƒ<?±úëC/Ÿ¿›V)úœ¶&?åçÐ^QÅ@˜gu/,?ÝZr§½HË¿åǞ¢ŸÓ¿è¢ƒý†(¿ãδ˜ù`ª¿â~5ZTà,¿ïÿ»lR8²AGNbcuTXS 2037-172?ïöê×h í?Ip<2ÿò?)—è8zŒÌ?:˜C§é½?Mî¨SÎò?Gˆi•'žL?ïéÉUQž·?g)²À)ûÐ?,ôôÈb.œ?9šXŒÉ–ï?dg[aÛ&T?dë̈́´Ûl?ï—djZ3J?'K)Èöu?U¶ý"±õ@?CaËN:ŽÃ?‡p¾´Dæ?'1Èg…_?ï\ß:??U/ÈYW?/¶šoì‰0?a˜‰)µR?^Õ¾@H–±?=ryIÜ$ù?ïìgøé?_Ð3¦	î?8Úwo&øö?10ííÅ,?`}¢‡œÉ|?\›ë¶'Æ?ï³'ß)?…î0P©Š?AïíñÝð?PØQ†®?'œå±¦¨?…A«4æUy?ï8ò%ÂÝ?Œ1þlçeÔ?dŸw E?býc¸u?–QzkâïQ?‹Ôzü¯?ïÎrõý?`"?Zó–?I¾JMyq~?7s]÷'áï?uŽ»Ìù³*?^;RÈ"lAGN4FGL J2041.8-7319?î¨áfÀ@ÜL˜_À:¯UQk,ŸÀ<•íÒt@ ò¾Íە'?û0íÕ·?È''·ÿá?»Q'ľ5…?ôÓæIîa?ù§zÓZÛn?ïÜCb¿æD¼'Âåÿäµ&Rz X¿É]F,4;q¿à•t;;?q¿Ù^¡IòAGNbll3FGL J2041.9-7318SUMSS J204201-731911?ïÓ¦Mà^?l$@)¥e·?-Î"é;³?Úá"Àz¡?u>…¿ü"'?k¬L1ƒq?ïzì¤ûÄÔ?…znb¥ú?g´œë5Ö?i¯¿õõ¢E?‹~銵µ‹?XAa«Šî?ï]$ÃPC²?€'y"ç3?a‰dFiY€?XâƒR7?'*;in?€!eülK?î!ZoÚzØ?"ü$*)D?'è¤×¥?czMÓ
g,?©0/ý˜Ã?ƒãŸNÈ?H`IŸ?nžª×\?<è GL?.ŸÐ<IÉô?†µ(ÛaÓ?†œM¾N?îffW^û?¡"Çëà?{ºÆûՋ|?ƒ×rÃ?¦"A¬õKY?C7A‡á?îÈeôÈá¨?o)CöBö?f¶"-Æ°?_–aïç?¢8pízƒ?üc¼ˆŸ?êðSF›gG? óiG+?•«±âKH?'óãP<?Á‰<ª*`|?Ÿ('Ã;ÊAGN4FGL J2041.9-3735?·X±÷"O¥ÀBž FÇd®À:qíâÇ
À<j+…¿È@ ÛB±Ux?ÿŠ7/+?»A*—®2¿~À!´(é?ÃG¥NX©@‰}G(ˆŠ¿íÖ±v/?áµü`äs¿ášmÔﱿÛSJÕù¿äh¸@"ÚË¿Àr€óZ€AGNbll3FGL J2041.7-3732NVSS J204150-373341?ïßr/-¦=?ZÎC)}V?AÓáÃ(k»?0É÷'Ê?lØA‰²þ?X]Î4$xœ?ïÙyã"/??p!êÈ¢¦ø?;H´»?E9ä´ìL—?q'©Ð'Z?l­Eé
^?µi{?pÈ×[Ïê?]5ºgë"Ç?Fû÷{Òú~?‰Xh¦ð‰?oßç^,ñ?ï†C¡.¨?cd%LÍY?`†Ho??ÕÔ52?ŠnžsŽ@?b.S}R'?ï»õ"Úxe?p_š–+‡?Uhaxuô'?G π Â4?|«%TB¸d?m/[…]\²?ïpÇ 4ŠÄ?…ßÇ^†?RäùHº>?a."–^?¸¼_òLò?xÞjq1?ï2Œ¦…Õ?󿌓½à?f spð˜?UÇÞô6p?–ê\ÀûQR?}窰'"=?îØSŎ?3`Eã(¢?rŠïI†×)?\磿Ěß? -¼ånÇB?}ŽPPR_AGN4FGL J2042.1+2427?Íå¡ÅbZÀ%'Ó"wÀ9åÚ rfOÀ<$;¿É¯@ y2&ì±?þa8"œ×?´›m"<æ?'vx_ë¬?àØ¢mþ‹@JÝîZ¿èœf2d[?ïÿ8Yã¡%¿ã7; ¿þˆ¿Ô|_Ìï1|¿ågðßьO¿£a+'AGNbll3FGL J2042.1+2428MG2 J204208+2426?ï%V£j?8>ËmØ?PdŸ»iqŒ?Cüh<h×ù?Ž*'ØS??€T.Þû?"Ãá?‹½•ÕÈ?>	Ç@å³?L(—÷lя?ÞcCp±?Š"åïkY×?ï*&]ü?…¾ÿ-ô?j­ì¸~¤ß?f
ӞÈ4'?˜æ}'<Ñ?ƒ¼êCº›Æ?ïN¬¢žr?osHß?r=¥Âe?R´Û	=¥Ú?'¢ø&Š?jPÆ"*û–?îê–)gû?'ö"–é©?fDÖN£ÍŠ?`Òm9ƒE?Ÿä¥7…Èï?'LdÛÂv?ï7#'2—#?¥ë£]¯áï?RŸ'ÑP÷?bWä&]rY?—ñ—•/?¥©''æ½|?íÉaÍ]o?šý:&79b?{Ҙw0g??s_™'…?¯ï"ûÂ)?™nŸÝåÕ±?îlBZ1h?ƒ›T}…dÍ?"™ñöUpñ?k­Õ=òw?¤]Þx2ü?€öӘ°EòAGN4FGL J2042.6+1629¿ž<{"˜À/*Îî<´À:Ä_½Õ¹À<]JÛÆdÔ@ ü›nÛÕÔ?ûC«Ë]a?Úù#¢œwš?ÈÜ!>6?÷€¬¹1@[K€1È¿ïøŽß#?ïÿt¿Å}M¿èJR]¿ª†ÁáÈm©¿êU8Á'‡?¹%ü"äÎÌAGNbcuNVSS J204242+162910?ïÇè}ò
?q"¨÷^?NqW͛¥ ?DžÂDù'?x=–&³+?o8ú¹—U?ïÚv½] ?t³N"¯ Ï??3OÈ ?K8Z¦Èz?pÑpÚåg™?s "žRÓò?îøæßÙ«?'4®Aù?m|at??tõYén;??"vŒQÇ?'{j•þ?ï9(wÐå?tÇDJþC!?c4ÿ¨wœ?Oå_¡v+?–tQ!
É?tV.Š?N—<È?×_‹…m?XÎç±åø»?T¢fô¸™?…'b"6é?|×ì¤z;?ïŒqà¡Ò?'ó[U0öý?SæÄjážä?jŒHôø§R?Šfßò"=¬?'5¨bÈË?îX¯Õ"å;?—•ˆŠJÀ?uËfF¹(|?|!A»+¥£?§»•å&'B?–ļ2ã?î-áÛZaÔ?'«ÈO¢p&?l2>Pә#?g#t(Îç?«^¾bŒù3?'†ž©ÉŸAGN4FGL J2042.7-5415¿ÏŽ6ë_ÆÀBä›A9†4À;G™Ò¤}"À=<ßP]¦@H;®@€"d®ÖB?Ñãz¥vÈ?ïÿûB«÷@FøðAF?÷'ïUÑ?í#Þ¬s;¿ˆÛ^¿‰¿Á–½FG.¿ëŒ#>Éik¿ïÿó€?ÖZ?î€Ý`í²AGNbcu3FGL J2042.3-5416WISEA J204241.98-540925.3?à5g{i$?Í
î-ù3?×´«k±²s?ͦîOî¼?¿'xÅí?¶ë
©± ¿?Ó/'^ØlW?Ñ'¿¬Ó³?â‹júS?ÑLˆI^Ì?Á'ƒ–fÎ?¸•ú`€^º?ØìM›"E?³¸5ÆHiÊ?ÙúÒIZß?³ã"ŸV>?Ê3Y$D¿?®D稪µt?җhuùñ?±Ɍq*?äÅ1ÝâŽ?²6"é^?®ñ«@š€É?Ÿ¸W'?Úî˂Ób?˲³j"ã?Û¢ÁAdŠ?ÌXñô#¨Ò?úŸæ1D=?¼^ 5
?Çþ‡YûôÙ?ÍH®qºNè?ä?k¦IÞÏ?ÑÉVíïԆ?ÇÊQi?Ã9táU?Ñ9[íË?´<)]{Ä?à'nÁ =°?¹zÕÐáæ?Ìï÷¤ç«?²ï_4?´Î¼ŒÉã ?¡2ñ¦ÃE1?ꍥVހv?°›t»ÖÀ?¶Ä½ÿ±?©%ÄÙºü(MIXED4FGL J2042.7-0155?é›8ýUÀ9iÂ;ySÀ:¶ãÊ?SÓÀ<_Öñý3@Ð3Xœú!@I:÷LÓ?ÇÐÜ&$?·vi¾µ‡â?ï:"£§@'èYp3Å?îò«ž~Û¨¿ê'ÇÅüÏ¿Ø̟ëÃ2¿ê3oce*&¿×'~!îè+¿èM?£ÙäAGNbcuPMN J2042-0148?ïj7+îÎÞ?…³Ã2ç€O?K.Æ=µ?:âj´üæä?'àᘠ—?…Xíý«R?¡…²m?%ŽÅ/:?`ky–\î?bܦ6vd?…C97D"ù?}8NúÞ³Í?ï5Eº§ä¿?ƒ]cÛj?p¡dó®e¿?pšlsp?•.ïu¦ò´?€¯ùVz ?ï5Œ}7Ÿe?p›vm¹y°?cq,'z<7?IÇú³»«?–àJÜ[ÛÕ?pë}]?î@²È>ȓ?oyz˜·?büxhöÔR?Vr¼L*]?ªÅò®\?ôÉν(?îù1ÝÑ4™?—"»4´?pZÂTá÷1?y+ÃÝÏÑQ?œÃ²Ü®?•vsg+?î8?š}Lå?–WÊЙ?}ÒbðÖÎ?y5n55–Ž?¨ÁºÚÍ?"PÝEé®?í­ñOl?Žœªí•Ir?w <	‡ë?g…Hìehï?±/†ø¥?Â/îbÒ;AGN4FGL J2043.7+0000¿ëãk´À8Â:îéWÀ:oÒ0¹Ü/À<\g=
¨@zî(½
'@n[þ-˜?¾¬ƒ×œ?›ñ"F7`®?àU'"W:@§6ycÄ ?î¹Ú¡÷Œ¿½Î6YX`ê¿é킺Z'¿Ý§]CýÜ¿Ú«zl­¨D¿ðAGNbll3FGL J2043.6+00012MASS J20434215+0001193?ï"%Çî?¬¬AýPx=?rÚĤÁØ?¬Ç|?¨?É:|kÌ?u+O»\i?ïÒi+4-¦?p?4	#?¢?@:igÇ#ü?D¥»¡Å˜?tÄK¡[]?m›*:«•w?ïYñy0?mYnäÔ?eð";1µ?c4ɬK?'¾~êçv?€ÁZ<‡Q?ï•ëbÔ?dE]Œ3
Î?\·ªÞ³Òœ?A¶ˆOL6Z?†î2	?bÏ	ȕ­i?ïU
¿²Ä?ŽÊ¶‹Ü†m?j0ôâ9p?a>
Hvšö?'‰s7®c?‹ê,4Ø?ï|ñÆΨ?Œ]i!¬£?P÷†XüõÏ?Xªç*'8?ŽÜÑC?‹‰=(š?*—"m?'€r—|Qî?uþ¨Òk?qˆ™R‰?¢Ä"Xì`?È뫸•?îÊï<ŽP»?€º™°t\?vVÈ;&x?cmU/"? †3/^:¿?~^½Ú${ñAGN4FGL J2044.0+1036?ïQeәo¨À30%"ôÇÀ:Ìóf"‰À<UcV­Í@8[ƒˆ?曥BDH.?Û`ØóK¼—?ïÿۂr5¨@‰
]Qï@
ÊMó(O¿í.Ýãö_?íSq+¼Fm¿æY©ŸK4\?­(<	E£ù¿ïÿÏ=ÀTï?Җ'ýCDAGNbcu3FGL J2044.0+1035NVSS J204351+103406?若Ž"Ô'?Žn…zOh?kSϞ*þQ?vžŽ¤ý?{Ñ€m‹?‡&Ÿ+Gå?ïÅNʜ‹?ˆsoè?^Xe5P§2?w½ñ쯩Æ?uÂÝÏmTÜ?~R¬?ìpõì´Q^?§—±ÃúÊ? Ð÷;Ãø?—`úar›?´D wa?£æ¢8‰\?ï3óŸ@ï×?ˆ©³ŒFY?YD"r/m7?U@¡V¹?—íIõ
'P?ˆ(dbh?ïY®/'`?œÞïˆf¦?;éÕ7$½?˜ò÷ü?ˆX"Žmx?"o^¶€Å?ïî•ýáJ?®lȓËê?†Øžõ1?£±ÝRîôÇ?'µÞ/?Ÿ
ú!G7?ëP[©ÇB?«KݖLÝ? gðklÈq?—¹®em<û?½I*|'‡8?¨
ŸUÆ0&?Fãí?ž‰Ûώ›?ZŠkN¼?c£ÊÚ¸'Ž?¤ˆIàÕ¶?ž|o¯hÍoAGN4FGL J2045.1-2346¿îa)¢ÞVÀAm_Eà´áÀ:‰ =!É~À<|µwE²@•òôÿ›×?þéùc-ÌÂ?ÂÉë›ïà"?¶]΁¸1?õ`Ɋ"?ü˜k&ºó¿ïÚÍáŸÂ©?ïûû…Fü¿âµQñd[Ê¿Üè˜DÚÐq¿æX²é̷Կԙ}_QIIAGNbcuNVSS J204457-234643?ïѳtó-E?d{ÏÀ°Qr?Aby(ò–:?0iÁ¡œkA?tùö?{¯¾?c¥g‡ër³?ïež¨!FÍ?Šw`sXk?jž
sÁ{?jl¼ïR?ðÓO8pŒ?‡(õA¶Ü?ï÷ˆQ¥?sj¿a`_j?a¸+®AÎ?Yâa6	R?‹ýàL?qXÞ]ÙÓ?îZ¶+u¥?¥£Â';?ˆ`~ª[Üë?fì‡ÔÕlÊ?¤Fäò±®{?~‹<)ir?ï³kÂV?rF©+å»?S¡ÿM¹U{?Eý`^ˤ?€°Ï…T¹N?pÜßù$O?î"9;h"r?¬†tH³?`?€ºãþ!7?ŽubÉæ?©­³M'"?¨3e*xº×?ï%ïŒP—?ƒz—Qg'?l¶ªÃ'â?jR‰¹ùs?—¾·£T_Q?€mšw7Ž?ìBTn^?–9å'dïz?˜"½ê[Óæ?€œc-á?·Ì-$?""ŠßY¦ÁAGN4FGL J2046.6-1012?ä…ÌþÔdyÀ>1Î_pÀ:ÀÛÉ¿ÒÀ<sÏÃøõ@ 33Yæ?þ†ÃÓÿÆõ?Å!#ü‰}î?³Žç á?ëjÑ?MGÜ?ý¸]ϓüw¿àDÝ¢x?ïøðâUË¿âó[Ao6¿ÜD""†ã¿Úþ;¤ñ¼p¿åa8^ì¢AGNbll3FGL J2046.7-1011PMN J2046-1010?שׁ®J£?­ˆnP¥î?H¹Sÿ»	?wkgŸ˜*?ƒU?ùÈ^û?ª›í¼?ïº×ehJÓ?x¶ûsæ?PX¾eþ?TW^͟?~~ÆÉ*f?uýiÇÌ·?ï~rX¯f?yÍËè²Ä«?^Åî`Ü?V<5{e?ŒŸq ³ç"?x±Õ}²÷¦?îú'¶é'?qö~Èm!®?tzí7ü+?Vùj0h²*?›íùm>È?p£ÎdHi?ï¥Þ^D®Ü?{ŠÙb\l?PzꏀW?Cýo®@÷?"y#³…?zvOÚ·/Ò?ï»R¯ƒ?˜­4e¿3?brøfÛ?h¬ÿfJâO?šû:>,oü?—º{̈́A?ï+S¦?ƒ¿›—ëš?cå5|@«?S¦«tÈù?˜ù(ÓçQ?'‰
£BŸî?í ûzà?ŒOÚ 4?"‡ÍC‰$~?q_&üx?°g*€ûö®?‰÷òÃÁOAGN4FGL J2046.8-4258?ïþ@Vv,ÀCXœM©?À:Ö0Ï«¤^À<"üæp@>M(|ËÙ?þ>O%ØÝ?Ï]JˆåAc?њýôþ@:'FK@
ٝëØ¿î·3"Hø?ïý̞ÿŠ¿ß;!`Lò¿á9ýñ7¿ê]ß3á¿ØâÏØðÇ~AGNbll3FGL J2046.7-42592MASS J20464397-4257134?ïÜ,ùT·Š?|~d	kñ?FGÑõtßà?Nå«'¥?nAaÞïž?z+ËJ?¹?ïÙ)#öæ?r
BFº±?Aæ…X°Å¤?Kd÷t»ù?q;šµÎX"?oïz?î~`Òu?žâ_ؙ
÷?Šó˜`A?¡‡;Øz(?¡]ïX"?š•È'$ô?ï¸CXÍÕ?[-yiß%ð?Zã[O¡å?@÷ÒDÙY?}%|ÙÊØ?WUCÕøŸ?ïÎÁ—m" ?xËâË>"?\¦áj»x?_ÛA'ý±?q{
pY?s֛'Ay?ïz4>vn?ÔœîÆnO?X¬2ÿ(æ
?kèc·N?Ž]j‰C´?Š0:Ðù?íҎÆèîR?¥¿'Ö?œ—]¦ºš?Žm:LR?«oí»¿:;?£\ùÆE˜?ïeYýçÞ?sˆrfºB?eÌ7àC݇?T§p¡º
?›9JÝŽ?rZ¾÷AGN4FGL J2047.1-7400?éæÇâï#À@ì4~ŒÍÙÀ:ê»±òUóÀ<\{Xeò£@‰)Ô½\@Ü0ûJŽš?Íb@<??ªzK[Ú,˜?Ù0ù½EÆ3?ø¸+Ë	ÿ¿ïhšˆ¬âL?ã"×/Û¿ë΅¿G(3¿ÕµÔl©¿ïcȑԩ:¿í¾ÎaÍOAGNfsrqPKS 2041-741?ï°îD–²ß?‡îvŽÜå?P¹žÄ<4®?Mß–êé?­;ëI‹?†úìÊâõ€?ï‹Õ)xÛo?†¨¾r
…ò?dÜ)sQ®?n¬ß-äË	?‡Ó«B¡UÊ?;(°Ý\Ú?îU¸ÍLµ¡?–²E‹E0?…¿äàS'?…	+'#Ë?¥4yö^š?"Zýzà3?ï)ëðÅX?x–°š·ÝÅ?/–é`?e–ýƉx¥?'+"‡ºR?sŠªÛæ¼&?ïDXÑl2?"'»?`"m£«W?]%"g=?h?•dX %Úó?"µàŒÔ,?îéà6"š?§ÒÈTçÍ?€=Whû
?'ó=H½?£ÒÊã?¢Íõ›Ê?í±N¦ÀÒ?ŸÌ7ÌV!£?‰–È­#&Z?ˆ§'ßoœ?®…mk'F?ÍË>F%˜?îÿðiN?"–=C­Sá?"íõ(›©?ƒ1ónk?¤‰*ôP?B0ÀÖäAGN4FGL J2047.9-3122?ï`ýMjŽaÀB±" ³Ô®À:bý%Z-À<køIRYi@jñõ%["?ÿô½±§?Äݑ€›pß?¿2&˜Æ
?úMn³<@&lXÁ?ïüšà–ƒ:¿è"@¡°¿Ü$.³q±ô¿Þ$)ªô4ñ¿áq¸¿y¨
¿æ^Ê@*'{AGNbcu3FGL J2047.9-3119NVSS J204806-312016?ïÉ°c=D¸?€m=ém3	?fÐFˉµZ?€DÜZÝ?oUеó>?]Ÿu<P?ïºk>×?u@ÅÔ[â?NÖÐgê¯?QxϽ̍?ð^w±Ÿ?rû')ïÐx?ï‹!Äuæ6?rœ¿vN?ZžÁë€?UV|A!»ð?‰ô;iÊ}?q*Oœcæ?ïXŒ'9?h´
<_‰?`²åìh©y??¨æ÷
:æ?'èÿÇñ§À?h6[Ïé¹?ﮓÁ	ía?ÉY÷Ùp?lŽ˜¡…ý?Â:~W'?znÓ8Füg?kj	˜‹ûÂ?ïCŠ]*lT?‹¹‡;AKY?\Úh;´©C?c"@'XŽ?•Á
Ö÷*ì?‰´1d?ßX?ïŽâ"R?‡ïg›3'?fcçDÃ
?`
î'Sá?š*°­²UR?…=µy?î6) ¤?…#‰xãaQ?sf,T¨Á?\nLb#ú?ª0¨kþݔ?"Á8\!oæAGN4FGL J2048.6-6804?ïÒ2t=áÚÀAì¹w…r›À:FNEÞ1À<w3Ï:eW@[9ë3?H@êùÞ}Ï?ºÃ¢Ÿ¨?¥4V@Jë-?ìŸóOîU@'Le¿ïü">`¸Ò?ïú³ääò¿èbªºSM…¿Êå9ñ=o¿åãflE£x¿ê.ՀzŽ¼AGNbll3FGL J2049.0-6801PKS 2043-682?ïêæŒÖ+Š?W?±s?6i1Ñ&¾ä?+ÇÁc¶e?bLM=i	?U©Ž€Í?ïÐú"'?wY¥«9@?GKÜ#$¶G?RUº¾J²?t™=¥fO??søÏ)á_]?ïjô¥®Ð¸?ʪ"°Õ	?c:ò9Қ?T%¼s'…Ñ?:
Åð–?~|;&Ã?ï£Ø VÑb?cKÀ¬Ý¶?pn;eC¬?T5íTY,?}¥´ºDO‰?['wœ¦·¸?ïÕÊÿº'??h9ÕÁ—X?L÷Ðà­×?DI'‰3?q{†!Wi¥?e›S|ڔ1?ïaˆè`?õ?•8þÚú?Z›…þ!O?l¢_•®©Ô?'%*¢d;?"kPK–@?îðb°›¶!?Š1P»X?qJb	lˆ½?nŸ_ã·?¡nM¡°?‡`/"~ñR?ï+FÈD?€Šëª(J1?"Œ,Þ*NO?r`‹¸ßÊË?X »Qô@?vÏ ÐqAGN4FGL J2049.0+1647?í­vµïÀ0¦ˆŸsÀ:¦ÖŽín-À<C瀭9Š@,»h zÊ@¬Å@'H?ß;Äý ?—ñ`CÑTá?Øó÷ÿ*˜@	è	ê§?îÐvoÈå·?ï˜þý–ï¿ãÿ‹Á>Ï¿çWÌ'ãt¿ÖâénÄú¿ßq+{ÙÀ%AGNbcuNVSS J204902+164727?ï¥d5‰¤¯?w\óÇ°?PbË{çˌ?AeŽ÷ÊDA?"š™9pÁ?võ^^(®?ïÔ;ž"?sGêàÁâ?@ffþ‹ú?DüC=%ÍU?sÕQþ¿Öø?qမ¥ß?ïD
Qˆo?6ZÒ@K?fÿ̉r
p?\Óä¥ÒÔ ?"ž\<ÿò?€G¿mÁ?ï\SJÕù?pºÇ~XÂ?hàAd÷jù?S×O¸Êc?'YŽŠÉ|s?nèü'¿4?ï<%H ?ˆ£#""j?h^Û|óô?[ß½+x`…?•o~~eT¦?‡I¾EZ?ï–àч¥?ˆ
@U¥?R¨ufÛX?]ºL/Ž?‡òíI^?†ª§ÃYÚ³?îL5͎¶?–[¦°2¬?wÛ¤âË?qc»ºÎl
?¨A.¡è˜f?"WŠƒæ¤Æ?î==gÎÏ?ŽRsNÞÓ?¬'™ñëW?r
{íLü2?¨6œS›#+?‹øØ~»AGN4FGL J2049.7-0036¿îט[)ƒÀ:`Æ÷ µîÀ;ŕ$¿ÒéÀ<³YÿOÖØ@#­ieIZè?ø–þ–µº?ɺˆç𔨿¥L9iƒ&f?Üi•ûg¿@ßÇÓ顚?çFyáîG¿ïÿþøþ"?ïÿÿ²}@?Ä/Mu~²8¿ïþø?ïñ"b"4AGNbll1RXS J204921.6-003930?ïuçóˆ'?'X_ßÛê™?O¤¨v~å‡?P°°ñ&ÙÁ?`½½·Ç\?'	²åҎ?ïƒ4gæ™'?>DŽnP?b›ªUê?l{ 
ÝX?ŠŒƒ_Ù?R÷/:Ã?íÙG ?¥Bz"ÓF?yŸ'¢>QG?€Áeªò?µÁ™tæ.?¤÷Ѻö +?íj+ù
Ëê?šÏ¸$ú)_?b8Bþ'ö?XŸžj]œ¶?´Þ#Š"[?š…tƒ"m?ïsÛ;ûXÑ?'ÿ%¬»I?\H?(ó¶?aÍ•é?‰'÷äÕ7?' ¥J¬ë?îÇÄ-?­}HI'¹?o™šÙ%CÞ?…(Ãñño?¡•Tƒ˜ƒø?ªÒ^ÉChP?íTÕwkFu?£M¹›g†?v‰¶ìŒÅ?êÝe¬À?³ð¸Ôç0M?£8ˆsÐ?èh»<£ì¦?µ7×ÄJèÊ?v´¡¢D•‰?zXkÏ '?ͧmþÇVý?µ=…€3ÌHAGN4FGL J2049.9+1002?ó<À4µt'yèÀ9FÛeNÀ;×/(·Ä@ÙƐȐ@'£}H*;?±âò~Jf?¸)ÙBQ@
£ì¤©(@h©ÿ˜Q?ïøkK¨tÿ¿á­#ŸAyG¿æÚw_²íþ¿çL£FÁ…q¿ëC®á){$¿ïþh@0FÅAGNbll3FGL J2049.7+1002PKS 2047+098?ïÛU9 È?hÄç}㒯?[ú"šXŒ+?Z¹Œ³Â?f­µÍÝ9?`çÿ1¾³î?ïÒ
ïd)?vïØÂݶX?Oæ)ø<®?WLäÔePq?sA€‰ð]?s±	UqÕ
?ïyþ³«B?"\Á4©?wÍ®"U~?~§æë/Y!?…™|8@Öb?z¥¿…"&Ž?ïqя1ê;?gõ…ZIÛí?uK5ϗòÃ?U£Ö
BŒ?ˆæJYŸÁ?bTQRý¯?ïšØ¸µµü?
X·éÉ,?s'hμF?pn¼±V»­?:ð|as?xèE¿Hõþ?ïv±©?''µb´z?m½}Ô3ï?±Êw»Øô?Šä6QÉìá?Œ½ºIã/?ïZ÷SŠ?'6Å
ï?‡íwLî?‰½ì¿n[?ýå`¦å±?"Éæ#Ç?W@#?ƒ"'cçPr?ŒÁB¥Ê_?rþ¦[Å]Î?ŸJÔ"²l?~!(kË×AGN4FGL J2049.9-2453¿ÕYË8ÀB¶â—À:úÎû{6À<_ü@WÞä@´wWû>¥@nxžwNì?ÚÅ>c?â öàqšL?ïH'AÖ@xh"<]¿ïO>â=ø3?Ô_ÀÚÑh¿ÓñS)rÀ¿é{'¾Šêª¿ë{H`A^?ºdÈA!ÞLAGNbcuCRATES J205011.52-244811.6?ïã^xu!?mT¢ßµ}?d¢§èmp?`$xžb?†ž~rÜt?{$åïí™?ïwg[•
T?Ž bžž?k±@2€?ugŒ¸&û×?‹^|¯upg?†ñ\gù¨<?îYwXã,F?—ß™VslC?&)¬Ä2?ˆ{X8³ø?¢UužÚτ?"fóaނ²?ï	o­{,?y|F™4Îx?hhɖW1ú?O'o '­O?›Äñ*1ÿB?w¤`úÅ?ïQ:ZCî?"£;Æå+?vs¯è—?oI³Ú
î‰?™Xì¿×'?"/<&΀>?îpX[qüÙ?ª)"!ϒ?€¥èû'?"+àa1ѽ?¤ÑÏ¿-m?¤§RÒ¦Nµ?í0ŽIœ½?¡éf…vö!?˜!é­Ú΀?'Bá'[Ö£?°s|b'ó?ži?MÝS?í}n±@'?•g!ªÓ0r?sÒ]ù7q?d &îv?²×d˜Øié?"ÿ¼q"ÈAGN4FGL J2050.0+0408?ۜ™Ïۆ4À7ùb¿ù'À9r{'pÖ,À< ¢ûB+@\Ø%ñVD@BÌ}òt&?­I¦èÃ?qßKäâ?ÅóH6¥ƒˆ@P5Þß?Æ{Pða§¿ãOÅx¿å›Èé}±¿äb\¶º;Ñ¿Ü]/ñ_SM¿ëçZ¢bëÞAGNbll3FGL J2050.2+0409PKS 2047+039?ïjyŽ"áW?ˆúÏC¾~}?V`¡ðÉô?G´m"sA{?'JÄæh¢?ˆß?öM?ïß©rÌó†?q	˜&ŸH}?:ï>€?E&.u˜?lø¥Wº¿k?o<Ϊ*?îhÄA/l¢?¶hہ]?tø'†
¯?u´i-È?¦Ô·vT?œí©ìA?זּèp(?aßÕÀÚf?`·1[É?Bw¤šâ¿?€ÎEüñ#5?^"ú,'>`?í"~òú3?¬¦Œ¾Œ9¬?s¶±Ðm¦W?g›_¿E·-?²(Iz½ù?«Âêîl¦?ïœ#rS#?‡€ÔÕ›Ž?JG¿âüŠ?ZÈø±9r?‡R§]Jµ?…}ùX…¢ù?ì
}ºôf?¬îK@¨ä&?ˆªeÛWþ?ƒŸ£Gö?¼h&HØÑ?«Šq6è¹+?ï40tD©?|'8\ŽÒ?uÄÒ ÙrW?a	%Ð?4?"¼ëlðÐ?xã=YÙ6AGN4FGL J2050.4-2627?ïðn9ïdýÀBbBAÃï®À:)ÞÊü5À<=BùyÔ@"»ªŒÖ@skd?¼‡¾ºÌ€?ÆÅÓ^a_A@
d²ú"¯u@‹j:±VÐ?ïîÀ!ß'¿Ð'9@=‡Ë¿ãKÈUnÇ^¿á."2Q‹ä¿è|J°j¿ïÿúâôAGNfsrqPMN J2050-2628?ïõ~®þýï?FûçJ",?@šˆkvˆâ?7œ‡!èÞ¼?Ij»"_Á?=_cgb?ïä@…<{˜?o@]G>½?6ÓÝGyR[?CDIÔ
Œ?häþí:fg?lC¹7K?ïy
vŒµl?ˆo
`t?t'mÿÓ?z!Xà–—?‡±ÎžÒ÷0?''×þ5ÒÙ?ïלý"Ù!?PWÑz¦‰Þ?EÖ=õL»?)¤¾'È?qæYË)]?N°^pJ?ïí^‡ä?X÷3^lhÿ?Tvõª•§?Qv[Ãt…J?QzM©+f?FKYvfz?ï¡3£'??…èyŽ|Ô?M.±F_m?f9엕£?…àPÑîc?"Ã9uù?ïI]Iº½?Ð	Íq(?ƒÓ)ñµ¡?ƒ£Q…,ü?"-ê¼$r¡?‡‹Ñ0¾÷"?@†?k«·€k¿|?Yˆ½ëá'?E—8À{?†á¡H¤.?i´qN[^ŸAGN4FGL J2052.2-5533¿ëËaè¨KÀCÇÞP'ÏÀ9M™æÆsÀ<-º9LQè@}»ÏN‡M@
hn~bÜ?§$H£v«ó?±ÒbŸÃý@$]È23Y@µ9"÷ƒ?ïÿ…]S˜¿ÛðŠ!«¢¿äÖ¹µ˜Ó¡¿äf;Óë¤ÿ¿æßyýò߆¿éà CAsAGNbcu3FGL J2051.8-5535PMN J2052-5533?ïòH­vxá?LKE†9¾'?§³Ú$"ð?	Ý%'ϼ­?Yô*ØB?K–LT \?ïêƒ9[?hdÐZ?*iIâŠ%{?8nÈq½t)?dDè"H?f›m_Ñ
B?ï‰èàdëM?'ÔL‰Jµê?^ÿ<^ö?dW˜QÌϝ?‰¥àKp?Ø‰
ÿ°?ïúúOÅm»?)0"Ú 	‰?H'³¨?p•²ÏP?@Õ8M¨'?&¬üÄ'‰÷?ïáÀë(i?dÙ#ŠCý?&'ðVŽ?¿M›î<?m' &,¹Ã?d{⦊76?ï»]T³¥?'QÛЯà?H\®qöª?f›Oq˜KÎ?m;'‰LH?€÷\†&iÞ?ï#Zº$˜U?m~Œ·O?l±zÌÒé‹?mœ‡¡PÈq?—þyhä4?Ñ"iXÖ}?ïó.ËÅeÐ?Hüj9°ˆÐ?0ø"Æh^:?$(£—@×Ó?UdG±Ô%Â?F«{E}AGN4FGL J2052.5+0810?ÛÌX¿oþ&À6H†zØä2À;Ӆü-ãhÀ<ÔÔoX}p@#­w§Ši?ì6q¬?æ\-Þ	¶?ïèø5u@Ä	_$RÆ@Êmˆn£ø¿¤	àmW`¿ïr}šàl¿ïj¼Â´Ž?ï÷V¾}©¤?ƁWƒt"¿Ñd§I……AGNbllRX J2052.7+0810?ï5™msv?šŽˆk^÷?Y.7¯ùú?V±'$M3Z?—¹ì'"T¬?™Ó*³'¢@?îÈIxw""?³8ûfS^?€k:Æ°j?ŽàŸù–?®?žÁ3‡.›?±ï[4ʆ"?ítšÜ¸?¤ÅÄÎ`y?yv«‰ÚU?}›¦z–?µ"Ó½†ý˜?£ý^–"Í?îªÐ‰Öê?žK¦q™Ji?XKù"ú)Ÿ?^甞
à?­òó1xc?ž3{¨Nž?î"÷žæL?«?âÈê?{/ØÐÞÅ?"'O˜GÇ?¤JŠú°ºç?¦ñÒ Û?푥	?ç?¿o*I'‹?'Ÿ.×á?¥w|‡fÆq?®dßÈdù£?»üia\U?ìV6-——?§òߎ£úÏ?yxÒTñ%÷?€wv¾h?»¶Án[
©?§²æ]L?énئ?¿8ý™ë›?{–{ùëÔÓ?W²L!?ËçèSˆ`?¾½ÙûðAGN4FGL J2053.8+2922¿Ý°› §LWÀ#´§qÉpøÀ9[¡ÔÑ~À;½Ca~ @ ïû_‡O?÷7קò!ñ?¹e1³rí?ËcËV€b@ÖKìgœÇ@	äQ»ßi²¿îâ/àm¿àÜ ý¦‰l?мj^ÄпÂåр´¿Ù1:_¢Qú¿Þ³+;-CAGNbll3FGL J2053.9+2922RX J2053.8+2923?î­§AD-?«gq]£9Ð?‰Ì¯fd?Žñ,á15?dÀZ3äD?¦a"'Ù?î'Kޔ2?±§¼Sû!@?nöÿ®?~uK)˵³?¥ëÒ$M?°Õ yëP?ìeÊgËI?§™Í
gÜ-?«T«£¾S? }ÞÌ*p?²§W]º?¡éó³O&?ë3á—<О?Ÿ1c»–b?{.fx="?bzãì'Ï?ÂWrÇ?ž€L-ºA?ì×1'â{"?¹J¸Š©?›6¶X=Å?œ/íã$?²f:9v?´ÁdZÒÇS?ëÚíl³??ÅP]P<?ðÐæv'?©n\´Hâì?½$Øg	Ïb?ÃZKnæ¤?ê½rð@"?­æ<O/ Ô?³\€­ÿ?¤gõH@±?¸¥"»È¾V?£m—ȉG?åïîžód€?°VÑø™=?ˆlí1ʧ?yûýe˜?Ó\»VF¢k?°b"AWê÷AGN4FGL J2054.0+7024?ʂtËL$@0cجëÀ;½¾<RÀ<L™iÈñv@ 
<ÿdÐ@í-zŒŽ?ÅÀæå|Ç¿èhV"ú?ÊkÅJøL?󏐬5'ª?ïâp½Ø=C¿ì€"'‹á¿ÉÕ`ÅÂu¿é"²a'•i¿ßdIÁ1濧ÔŒ:
"AGNbcuNVSS J205350+702404?ìþÀ§qëÍ?ÃVvâ¾d?Û7ý%Ý?Ág."Å›?°",ÆE_?´RØ)4GS?ìýӍä¸/?¸RC¯šFo?Ž&!–—ul?'´!Ýμ?´LŸ_Q*\?¶÷ ´5¿?íóYN$ü?œ.ç@Ü?…^sݑÃ?†²õëgD?«rÎ](v­?™D'Jyt+?ëÒ÷éR‹à?–ÄPu÷?ˆ Fm2ï}?qÄùËU¥?¾T7éëŠ?–€p捌G?ëAÙǺ?¿þ3!?–?‹¯2|æ©?°_U=-º?Áøpé]b?»vˆGŒ±?é6ï©?Ç'AÚt? úêϕ?¤Â¼>ê^t?ǸƒÎšñø?Æ7ºÎ¿ã}?ì
òÛ1òõ?ª%lo@µ?'…"™!?r9ÿU¢?»aÇÆ'Â?¨^ŸñÃu?ä(•	‰c
?®ûœ »?zexŠY?'ŠGÚÁ–?Õ×/"ö¥A?®'ܪð–òAGN4FGL J2054.5+4731?ëò¨¦Ò½'?úG-ÉÀ:|sÁ˜¼$À;àý÷Cõ@"
d|¬Mü?þÆ*\}?Ì1°|4.?¥&8à™?ØÏ1Ì*æ@¥4L?äæ†ý_¼©¿Äè'Ç¿ï³Ü:þÚ?äc=¬ˆà¿àւ""F¿äØ'sâAGNbcuNVSS J205432+473338?ã7·4gÄ=?Ér—8㘹?nF±¢÷Q¶?së¾cUJl?ÙT3ÁM"?Éi‰ŒíJ?çÁ:̞mƒ?̏|"æ8?rñ‹!ù{_?‡2þpcq?Ð1Ä:N|Ý?̽]vR?è2š•~=.?°ÉaÛӀ?…aaL~¼Q?+áW5Øg?Íß•?ƒ?°"Qª¯¦?îVvÊjP?"%3›VëÇ?i¯§¾›ä?]À"€N?©ŽûJ?"–~;'(?߁ìÂn¥?ÊgÈÕád?†Ä&'_?¨O¡æµ¥?ßÇò¶B?Ês£:Ø/?áè§'Õ È?Ѽ¨y¨¯Ù?€N´OÇ?¥£­91ñ?Û¬;Wnü¸?Ñ£T""½?â/nR̉9?·
Íã?"¸®?•'Ž?ˆÄA\M?Úe˜vÀ?¶Ü< À
?ë+sãÉà×?°XåÀw?ˆ¯uXY£Ù?†˜Fɘ-ì?ÁÇ9÷ϧ?¯¯øªÆôŽMIXED4FGL J2054.8+0015¿Ñü¿¤ÀÀ;äÚ	Ì2À:")¦ÂwÀ<O®‰ë¦­@!GáõRýÔ?ý!þ¨+¡?ÀY ãOp¿o+'\2¨@?²H`þàì@P¹Qð¸?嬗moo$¿ëåáℿÅf˜egÿ¿Þÿ²þ æ¿Ôâ5_wn¿Ú¢5_wnAGNbll3FGL J2055.0+0016RGB J2054+002?îòcc–l,?¾it8¦T?cïh ?'†XWx?ŸP¯ûÔV?¼š "Q¢?ï²1è§Á?€nµŒ¿?QŠlˆœú«?XÔ=,!ñ=?B84Õï¾?}0²–:øx?ï.€r{?‡Û‡Í)Ä?Zë¤úxê?`ÊyîPþ'?˜7vY¥?‡À£Þ;ì?îÝ-xf̛?y&8Mú3ã?T3&‹Ã?9øñ¢ÌP?¡Œnã¸v©?y<¯âÉ÷Ð?ï«/rg?¦y– ²P?d;¬žm	·?sÆ®‹}Q?šƒ)ÎW&Þ?¤H…ªÏL?ïC|"Ùžö?–Ì'"öJ'?Yîуnz?ed‰ªSÊ.?•ñ€PìXc?–n^JË?î	t®†CY?›S(*`Ä?cÙåÂB¬a?Z½ o+Èå?®+ºC©?›	>ªü´?쮽٦
Q?•ã\OD'?i'Eûp?X¯í¼Y(»?¹½‡
2?–·ï¶ÛAGN4FGL J2055.4-0020¿æX'´èLÀ;sP]¥À:F0l¯UÄÀ<<¥5¯@ ê&dä?ûäÀ>Ië?ču‰nÿ?´wÀÁP»?ôô¿%D]@Lyµùw¿ïܕ'2Ê®?ïú«bùÌ¿êRÆ«ú?±1¦@F¿àûã:Í[h¿Ù·ÿÛ<§AGNbll3FGL J2055.2-00191RXS J205528.2-002123?ïºÔ 3oL?t‰/]}S?@•½Æñ/¦?<v5•°­?€A|	hÛ?sÊö®©"e?ïÛ½d"Â.?q¢Ù­´šX?<C\4^ã4?EØàÁYäK?p]ý\•?oß}:}©H?ïz¨©?ÍH?+[p?qnÊ{^‰?xA~,-=ü?˜õŒ#…?‰÷['';2?ï/^Íj×d?x`+^±?gG¦úُ#?Q\›'§ñ?—+1mF™?w'kH2QÁ?ï",@êoº?ƒ"z4"Ib?Y}
êÊÉÈ?YI©¾Á ?‹ÅN–J?'¤I˜öÁž?ïŒB…$†a?‰OŠ©R#'?Lãò[äÒ?Y@L±Â?‹!Œ·?‡¼Ûç?î-'Eò±?˜«'÷¬ú?wiÜ`À>‡?{âzÅӒ?ª@PšvP?•Çíçe¯?îaŒŒì?'àE2`»²?}‰†à>…?qÄ	íÝ@?«…É&PÖð?'¾jÈñ'AGN4FGL J2055.4-0504?çjõ×)"pÀ=ÎðZpŽÞÀ:÷ÀªšëÀ<˜ëô°@•\­€k@ö¤¼ãJ¾?ÈWûØð?±*ð¬IJ?å¨D€b'?û/3÷Ô7z¿äûÎã''%¿Û•ýÈX¿çk(½Žkh¿ã'ßx ûŽ¿à?¾øMÚ¿å%:|CGAGNbllNVSS J205523-050618?ïÁ´ˆ™}?o'3Gi?;¶AÈou?(w¸<fY(?}¹A‡ŽD?nÞ8ÈZ	©?ï"ÄãtY?'êÎñ7`Ð?]+o"?asUÁ·G»?‡)Y<G´?€?ˆF÷?ïiÝÓ/?{ڐ)b_Ö?e4ëF˜ìO?Z¸0éÍ$?7à=®;†?yägg}¾?ï6ïw®?q°¦æ³!±?gx²"?Nõ'öÞ¿?–\m­ò/ø?p«¶†ã?ïi5å%oa?'¾9ß9Sæ?MŠ·Ob±D??ˆ´‰H,§?'ìí›ÒÂ?'Prâ@?î¨9ïžÅ?¡üÂ/{Gé?pæÂD'?|tzÑ,'ë?£_—
yðo? '‰Hàï?ïí^_(?†g])Ãù?pÛNø8?ejKBœœ?›šõQô?"r—˜&ô?í­ÿC[cB?d˜=Ë}ò?}x¤xè ?jî·'Öé?°¸{Ÿ…,T?D4x²¸1AGN4FGL J2055.8+1545?î˜?ñÿٌÀ2"f¥P‡À:‹Ÿ_¬8À<>À//˜t@E'Äë@¢e㉧´?ÌÕY8U†ð?˚KäÚá?ü=W(ÛÁ\@Rr{r'¿áëCII?Þîs恩¹¿çÆIƯc¿çv?!}ÿ	¿ïþadžæ
?ïô€ÜqAGNbcuTXS 2053+156?ïᖏgÖB?aW›Q½}s?UJªê¶?MékØ#6ñ?cãK'uÔ?YÊ$˜
?ï°¤Ýs?ƒVÕMɒS?`ÃF×ûã?kíŒÜ¯p?§¯Ý)óŽ?|ëq—¸¿?ïITèd­Õ?ˆñ'í8ZÃ?tØÑÕ*­h?v*–N;?'Ÿ.wðN?"ÎÖ.£Á?¿JX?l0CªOÐr?o@µ½º8?S¼i/öë?‡MÒ{w?gíÜ¢¼Ý³?ï»êýÂì'?x¿âI†ê¿?k:·%ŽŒx?gíý¶Žš?tm%~³ôî?qsH~ùJ#?ïw*ÀL?¤Äjߏ ?xÈü›è?"Ôq¤
 h?˜>Ûz='?˜Kb'jη?îÌÕeø']?'ßm6¯×ƒ?€™õ¢6—?}H"4Ðp?žXµz€?+2|·³!?î|å>Í?‹k²#ÕÒm?†Ç0vW…?tZÿšÊZ"?¢¬ºPÑÝ6?ˆ\ž·FÅæAGN4FGL J2056.2-4714?ç‡!‹@ÀD1&|k‹iÀ7Š8|HOûÀ;"K}¬Ô	@k?jyž@ÒΤ=aŠ?"'p€Eµ—?»|ûÔ!Tä@"Ô¦°)(@Â*/ÔY¿Ä>ŸøÙE+¿â›SíNM¿çX'AƒÍ¿ça''zï
¿é‹¤ô^¿ë4ÑΔM)AGNfsrq3FGL J2056.2-4714PKS 2052-47?ï½O<d?·Y¾Cd\5?v¡½Pj=?'{²ª–ÿÒ?™ƒí«²ú?³yjrÚ?ïšqãÈû?±•ß‡?_&óř+§?yÂœfÃý?…~¨')½?‡-`÷–Ãß?ïm$îÌÑÕ?'ès'¢?|€¨F±›h?…ÔHRecÃ?†vp%«*ÿ?ˆÁ'wßÛ?ïëµr_V?NéǁؓL?M4>R£te??¼\å*Ñ?Yúü_yà?Cåi|ºæâ?îuÇT½Çv?»w%.o±?|R8¯8…4?Ì±m! Í?¥C›PÌù?¸|gVa?îø{õ¢a?¥©–'\?tܖhìŽm?Š¿ˆ(@?›¹[­…Ï?£çÛmdâ?ïJd~@?'äXÚWù?—is?…ç71D›?ŒfRÍàњ?Œ ñb…,?ïʙ&F|?jñ"/ œ?c s½cç?X9.mþ?ž?q2œåwÙ?dl혏"†AGN4FGL J2056.4-4904¿·l¸Ÿu$ÀD)GA1MÀ:Õ¶;ÏÆÀ<IjÃQ#@Q/@4xƒ@QÈ"n·?Ù1ŸY?î+hߝâ?ÿoœp
¯@ñËß¼é¿êå¡z8«B¿Åö
³¸(Ñ¿é­VN¿í3oce*&¿ï齞[ :¿îíÑ9*AGNbcu3FGL J2054.8-4908SUMSS J205613-490415?éqZãGÚ×?ÁBÃîp¥H?|Áì4R??vj°{?ÉT…xþo?Á
2Ú?íe>·åy?´uê‡ø¨?¤réɶ+›?ªj"E"+?ªfÂLƒJÕ?£h-‰ý¤™?ìî¤l +?£Ýj±}$¿?™:HÑ*)Ÿ?z…¢Ùò?²<JdŽ[3?¡§^°'?ëp%Z¾£¥?¡èéêçU?©2x÷Æ?'GÅ坖8?·å™(ÆÍÎ?™T£›P(?å¡èDøW•?Ljd»Éø»?‹!VP—é?‡ËSt?Óã"ú€å?ÇJ¬Œ˜N?è¤	ÇKzõ?ÄÝÄ
Wù´?·Ú{Z@¹?½¹Â]KúC?Á'›4h+Q?¸Þ¶Ô†ã0?ꎎ(!\F?­ÀÞÏP,5?¤¾
Uù½¹?˜‡m±¯(?À–D
Øx?ªÞ¬?°ç`?å$Nü'bC?µ¸vO»Ê´?ºdÒ^ÿaA?«ÅŠÌßþ?Î<ZÞ6ÆT?°éô)KíƒAGN4FGL J2056.5-0202¿è™QgÑ qÀ<Ž¹¡vÝ­À9ç
›dtõÀ<:"ŒòÂ*@M@NN†@‰êdHR?»äC`ýÆÀ?À¼Ÿ9@>@ ¾×@Ä@I'zìZ\¿k
Ñ¥'¿ß*m¼Æð?¿çÒ·'¨ä¿è0¾yLòø¿çôÝøn;G¿ðAGNbcuPMN J2056-0205?ï¿É'{¬?³‡»UôN?RS"–HJ?‹Ë
‹çWÒ?{†{!cóß?±oz¾x{[?ï܅;¢†?pP‡³??"2?IQ—¤{ˆ?o—²nÁÞ?l˜Xmó?ï¢F÷`IA?|¹ŽSÚ»?_悊H?f'àqS,2?ƒå^ӚÓ?yccIöÓ?ïÉßW=ÿj?Séö©ßï?TE!¸ Û?4Û¶iôé^?uÿó"È?QÌñŠÇCÌ?ïçâsÁÝt?bà»s}‹?F¼~dà=?HÝ3j?bnla؃)?\Xê
åšÉ?ïluÅ»Ü?™áœ¿H<Ë?Ty[«‹U?dõ̕Xc?'0ß°zÜ?™@pdjX{?ï@Äòžÿ›?ŠøwÝ·§?mUPL?osÕfƒªŠ?"<· ¨?ˆÊ5¤ÄÉ]?ïhÞW(Ü?u
Ú	Q‡?lЊ‡†S?TÈ¡a솊?Ž"Vû,?r6s í«AGN4FGL J2056.7-3209?î[68'ÒÀC¯!JÓcÀ:ŸZ·ÜzÀÀ<G{4SÄ£@ô¨^•@¤Ø&"»?ÅûœÙj?³Úx±íxi?äú›qàíì?ý¨å|qÀ¿àh)µ/ë¿çóÂâæ¿äŠ‰Ü¿ïÿÿÊPË?ïÿçÁŲ§?ÀÍ<HۑAGNbllPKS 2053-323?ïÂÜê.åú?«»ÈR¨C?4¸cõÆ%?5À±ªG¬?}F¥ºçØ?«½€Æ Õ?ï—ÖG8½{?Œ›8ôöß?ccâšÂÎ?sF™•[}?…1uyñáï?…Ÿ¨Ž"¤?íâÌ
4F?ŸÝ²…ö:	?ª@Ñnš?šú«ìÓ3‹?¢þÂL'	?'Ž
!Å?ïå
Q£Ç×?_7Ôê¿Ý>?%·#»aE?5#òظ?j™ÀEgÚ?^ìæçåàÐ?ïœ%á¢-"?Œ¯‰^Ò¸
?E‹¾Õ'Û?AÑ}l"ÇZ?‡Ë¦ˆÊ§?ŒH-|v.l?ï8ÌؾÑ?¡è
Ό«Ð?gLT‹­P»?{×±;Ӕ?šo[ÔþNÄ? 䉀<"?ìʅ}éöå?¡õ•§sVL?œ¾;óÙ?—nÓ±é'¿?²|EÔ?tÀ\¬a?ï‰q•}g?‡	*§ò˜{?/ ÈÌ×µ?9·ˆ\¾·?'šF)ê?†ÕT{oq"AGN4FGL J2056.7+4939?ʹ7¢6SØ@	<"?¾À8c}}Ú À;i!Æ#e`@!p±E\Öp?ýMoõ[aP?¨³"?ãDÞ?¡=¢^6?ö­§%sW@	¦"Ö/?Þq&þòcà?ïð¦%™½¿Ëä¯A¡‹¿Û'$l ¿à]*"As¿Ô¾Ô;«ýŸAGNbcu3FGL J2056.7+4938RGB J2056+496?ïw—c‰gG?‰ÛÛ³oƒœ?Fƒ%¿;´æ?DE2Ùk?Xúgñž?‰
!ú£5)?ëÈæW|,?¼×M¢RÙI?v'KÏY†?"Y
s,8?À'ÜCsƒl?¼œõ»û¼?ìŸÊÏWÒ¶?¦•GÒ±?dût³?ƒÿP4ý4?¸Õ
!Û¶¹?¥¦fL3a?ìe᛻ݼ?—•Ìc#'?—,…'S2?{›Šûë(?·Ñß²âÔ?"|¡4oR±?îkcÑ5½?¢»Q'61?eFæYîŠ?g@\F;öi?®$Û]‡E?¢&MóX×?ç1©g0Õz?Ɛð"'Q?Ž"Bº?ž¯³‡7‰ˆ?Ь˜ORà?ÅælÏׁ?酾ˆ:?±,œõê^u?‹3°®'?‹dCú×?È5ÌÄØüJ?°"
šíêo?èêœ*}Œ?¬tQ¡ã^?§ëçáLö?'pä |W'?ÆZ•"¶¼Ñ?©q¥8"(AGN4FGL J2057.4-0723¿î¶¬0Ü'À?P]…TÖÀ:'%üéË
À<Eí@
@o"&¾Þ@pHðŽ?›™#'"?ÁÉÁÕwì ?ùLÝF—"@SãÉ®¿ÏºÆdþ²M¿åëðž¹2¿é(ôëÏÇS¿êîb›Ö‹¿ïë[rž¿îߋ€Ò"wAGNbcuPMN J2057-0719?ïîDhA¢?S¶~"ñ?B ÷S+‡?:è̉Îä{?Z'e`Cõ?N¤rbR?ïtJh•%þ?"	.óu'…?i{wRÆn2?q(¤?ŒŽˆ
ÔY?'?t]j¬?漏T—?xúüÄÈ9?Z¡ˆ¼¬¸?Hk¨éšm<?ƒH9ÑÇ+M?xiF¶ŒàI?ï'ÕQ£E?ib¿VY`?q©z‹'?S¢2´!"?†{ÖÛ±{"?dÆĖc¬g?ïÏAÁ‡Ó?n…Ê)k‰?[º´͙Ï?Zâ<þÀ?qpÌû¬˜T?gT­ Õ?ît,Qšã?¦'€‰ŽoÖ?|uuˆŠ?††Jÿ¥°?¥.ŒL­lZ?£sAÖ%{?ïE¼C¬kó?Š…Ñ$p-Ø?k()KG5ý?j}³Ø´µr?"ãrh˜¾Õ?ˆy–ôí‹?î"ãfc®ž?ŠñÇuMs¡?‰ø›"û¸?tÓhE? 3ı(	<?…tŽžô	mAGN4FGL J2058.8-1442¿Ú
mó‰¶3ÀA`Ľ3ҕÀ;#jęødÀ<˜dH~ôÓ@ ¬ˆ0½7@u×ÙôÓ?ÄrvŽ*¦¿«;Ž÷T4á?æ!EÊål?ÿ'g΀¿ÛÔñhˆ¿äpÝî]@M¿Û%⽤檿ۜ–ƒå}H¿â~äw
}—¿ÖH'¶þ.oAGNbcuTXS 2056-149?ï×ÿ>þ²<?g
#ÚÈu?=£Æ`WN'?/$6-M?r&$Žë?e±«êÅ'\?ïòµOé³?"lðW7<·?\¢ÆÖ¡?`šˆc&Æ?ˆ~C•?™»|>?¢'+?tߤ*˜5;?Z±ŠåîO2?Aʔ°Á>Ÿ?Šþæe=J?twólIÛ?îïù"ìª?{	ߕé?aäÓá|)?E܍†Ä?ŸÄ3xÑ3?{_ÖýÄ»­?ï»Ø»9ô»?mûrH½1?Kj!¸ã?;ß¡/
mÅ?~¦^"
`?lÔڋôå?îÐq5]–? ^{Zp7@?eœ¿€–bâ?n2"ö<\?¡Ÿ µ4Þ7?Ÿ¦¹‹áy?ï/Š¼SzH?ƒ5÷|'þ?bO=8m?XÈϗKne?—ÄÀÌ©àe?'‡NÍ`?ì'b	"?™i?]Ò}?z /jÎo?ḣÀS?¹Í)ûas?™ÐïàçУAGN4FGL J2100.0+2103?¥ÉÇû$û—À0#æÿëÀ:‹DÙMäÀ<(6'cDs@1Þ ôp@Ž ¤»5Ì?ί¹<:ï?ÀâÔánD?õø¶DË,@Íé/.è?íÿí@_Á‡¿ë>"E]¿Ù ²ýî­È¿ë€ y\¸¿Ý»lb&¿ðAGNbcuMG3 J210007+2058?ï¯âڑl¶?˜v¬÷ȸ'?BöÅâoÊ?U¥¢±Œ%?'×݈C6?—6ñrU?ï·];'Èâ?³_=%C?UG{‹±å?`ŠV«w?~íP<»Â˜?8tL@h?ï!K>9C?ŽE¯§õ?qƒëÑWŒ?|´‰…Š?—uAî¾?Œ<aN1bå?ïai§¤}?kwéPP!n?Q¬dN•ƒš?79"&/?'¸ŠÅ'%?jlÎÃw?ï]žI_M ?"íÖ0Ž§?Q²xëÕ¢É?Q["9YC7?"1A'oÔ?">¼ÍÈ?ïP䨥iö?•Ô'¨Žö?f~"!'~?u0e<¤?"˜Š¼6F?"ù¯íL?íå 0¶m? lÇEÒ±¹?~L(4y?€ÝTóÍ(?­Üx5½¤?Ÿ<pœ2A?î9ÀLz›Á?‰»†Õüß?bßÉæ}ÌÙ?Q¼™T΄?«5þ™Âl?ˆ‡&]3x-AGN4FGL J2101.3+0912?ÚZʨý‡!À7ƒï(Ag©À:ã´+W€À<v*¦€2@ 25\XF@ÍÝ|è‰?ÁI¡¿¨ä;ÃS?åž6Kìg?ý¿SrB舿èÊ(­ž3\¿éãîâvWJ¿Þܳàֆ¿Ûú\}‹Ñ¿á¤TÞ~¥ø¿æÆÂâh?"AGNbcuRX J2101.3+0913?ïÐuÜ%/d?p¿¬|o?DÜ\ê,˜¤?6,'—ž?u)†@‰M•?p)7¢Éc?ï°FÑSM?~Qâ©`"ž?T	?Á¤a1?ZÎJ£"?xÆSª¢?{tŽÇ×c?ïx*'¤Nm?zʶÄæ
?_,±HÀÿ?XYH¾OX?ŽÉ%í2E?y;±Ð}́?îöUD³–Î?x'×Í¢±?eAÐ¿€?J–îÞãW?ž%löùF?w©+Pc¹?ï¤øŠ•Å¥?tñáØó?V¹™*Ht?H|<"͕?ƒêª>ë•À?sշՋa™?ï'b·|¥å?"fÉׇ¸\?e¤ÒwNŸ?q{SŽ˜?˜_ÆPãœ?'*"ë	?ï
aÕpE?†q0¡üÝ?d°Ïúf«?Sô,WäÒÚ?œ«N²F?…§ÏœË|?ìÜKº‡Ù?–ˆä'¢Õ?~âѕº4?nåÕB£O?·=	}T?•úЃJ(ÁAGN4FGL J2101.4-2935¿ïî¸Ù0ÀCï–AöD•À:pÜÀ<4!'÷¾é@ìò²°@Ƙã'4p?ÂNÙ¬Ú?ÇRÇ%Ãß@.Lÿy@
朌h-¼?ëR¼ÐÖFÉ¿ç.÷™ÿðç¿êí3¿Ë¤¿ç¿jäz¿ïÿþˆ0»Š?ïÿ¥ÂqÕAGNfsrqPKS 2058-297?ïî¾ÞîÈ?XŒâ­-ýï?S*¡bþ·?Pz–"´/?N°bƒ:?H[RzG"²?ï}È'w?þ§é5?hw¿º¸÷?ry¶1Ð;¨?ŠžçÏA"2?‰Ç£Ò‰x…?ï}ÝÖ+è‰?…A8‡ðt©?n
wæ'1É?rjúŠ£á?‰,~|÷f?'§@·¤·?ïÀJnåÎ?`¤Lc\þ?\oÞT÷?DDûE¹_Ô?x¾ÑVà9¤?\ž{nÌ?ïæ2Æ?®°?`ÏýVÎ?\ýa;m!?YV«~b¢]?V&ø''?PsJÝlTÙ?îµIÔ=.?¤»ëú «Ã?y 9O诱?Šßšˆ@¦š?¡w[•Í¾,?¡"qÀÅT?ï)®m~Å?Ž¼¹w?|ÔÀÒéª}?y€k•N?"•}=ÆÊ?ˆ/²?2?ï
ðGó?"û¶%]µý?|߶q?lŒëSR9í?—
/þy?y¹µ±èÇAGN4FGL J2102.3+4702?ïþå}³+?՝ò#žjºÀ8¸lD̹À;9•zP(6@Fx M'{@'ï[m ?´1[}æF?®ú	pìý?÷òZ
7'g@¼¾"ºêø¿Út_Cý?ïþdž;îÄ¿áõ
=€>)¿ãmŽä3ñŸ¿ã´ =¸g¿åálˆ€ÃAGNbcu2FGL J2103.4+4706MG4 J210218+4702?ëÁ"ÙÛ?±jßÞ&°Q?nýQÂhc?g›éG "?À}¸iµÈœ?±(ŸFë7?ãjy»c?Ñ>\&qƒÑ?‡\B|ûsì?™Åöºt+?Øp*²'§[?гK"ÁMñ?éI)zÞԝ?­ì¼´ÚEd?¤©iu?›H,ûœÕ?ÅÙïÑoÚë?ª_A7Ž?ë¯v›?—²ÿ.9r?¡³{‰aˆÉ?€óA|‰TÞ?¾hÊèYE?"1‡o—?äö'ª«Ôs?ÀùŸuž	7?™Ó2ŽêáW?ŸL"ÚÍSv?Ôu§¹©?Àq–ßï®?ß²¢˜à?ϛ'<ž°Ÿ?•FK,½çñ?«Àã?ߓ€›ù?Ï!DÑÉ¿?áÈx)åà"?¶p<9Rm?±«59:Ô?£Ëÿª< ?ØB^83g?µ€yˆPGË?æÐ#w"Ä?¦çƒø??±ç²ºf""?–°QP†~?ˢÅ3Pd?¤
E0ê6HMIXED4FGL J2103.0+0342¿ìZñ"ǺÀ:îÊFà!À:j;4¦À<=EŒÒ
ú@e`ïYÂ@¡¬Wâ?%?ƒo‹©?­Ï‡Ò?å—?¢,e@౫´#^¿ÜqÃL¿ä¢C çU¿æþ½c£>¿ãÛT"¼'ÿïnoês¦Á?é|ðKWgAGNbcuNVSS J210301+034411?ïº17zÉ?u£VA
Mj?Q0àzƒÄ?CƦk6©?~›EΐÑ/?t©'	]"?ï±tyS?}Ëö©Ž0?TŽÒº¦EV?[k
m÷¿<?Væâ'?y–'Ç^Á´?ïŽ"ÛHf?{"¹Œ³j?dþЧæ?hÅ¹|ÊÁ?‡7Åjã
Â?wÛíFØ?ï¨ÐñAÅ?d) "Q	?S.oË[/ì?8»
(ÒÈ?ƒeõªHå?bhŸrèz?ïDI'D?'– ÄDãÁ?fIòz£å™?`:M,#a"?"­ /â{?T/*…§¯?ïZ™'l?§ú"{¬?cˍî	o?qB
Ž­ß?œ{I#>ÜO?§}qc8?ï
òˆXÝ?Ž8Á¡ý>¥?pr±EƒR?is<Ãì?š$ûbÓ?‹F©_ރ?îâKÚE†?†®'_˜ª?o‡x/í¨—?\ÝyõG¹?ŸÅ°á¥E ?"ÞxÀfAGN4FGL J2103.2-2114?ÚrY¬Í0¨ÀC•_x5œÀ:ûXª¼ÍÀ<Ó׃	4@sS¶
"'@U>S!æ?È¿4ïb¤?£›¼£M¼:?Ûj•4°
õ?ý¢ë$PÂ:?ï?Äpݸ­¿æ\IÂkÊÔ¿â%!!¸·¿Ú¤±ÛYØd¿áœ?':z¿ïú"á%Ê?AGNbcuNVSS J210312-211216?ïÁ'K|o?iÒ\´,4?@ËŒº>?1ú?}Sd­¢
?i#mÞ¹?rX?|!å¹)m?X±ü¤oMM?X¿ÑïñÊ?…û	½R?xW¦éd[?ïzÂÑ¡Gä?sJWP´?a%=¶ø¯¿?I›w]1?ü2.ë?qúÄSÄ߬?ï)‹HëM¹?q.æ"mÅ?iKژuï?Ik	âw›ý?—¥iî3?pG\ç]Û÷?ï…܃¬¥î?{"p7'?Opܘf"¨??é¬ß'êF?Œ'ÑG\•??z¿aOáIÈ?îñÜ·Y%¿?˜‰–.dž9?hIÙs<x?p'z`'Bƒ?žÀŸá¿õ?–×[Àî±?ï"P®²õ$?'ô°b©-Ž?iC¯·{z?[{8xŒm?˜t-Šô?—œ:¯?í£ü~7µÆ?¸K ]ð?ˆÒYy"?fwPԜ$?°ï"±ã~?+Ùw«UAGN4FGL J2103.4-7816?ì™O"4LÀ@'óÜNôÀ;ºòù‡?ûÀ=Wg:¡¼~@M°À§¥v@,—½÷Fô?Øü>ª_º{?ïÿÁ¶ïö@—»=XP#?þΚ,f?ïغadw¿äz7i"ÙI?à)Ñ =ô¿çÍ˚¥˜¿ïÿßéà
¿ïÉöž'ašAGNbcuPKS 2059-78?ìvŽg¿à^?¸¯Æ琣?­8\‰`ü?°ïP!®æ?«^¼öVc-?ªººmÓé?â2×P¼ä€?ÒGk®¼4?Ó×zjªBß?Ð"ë°pSX?¿[ÏoЄ?¸çº™+{'?è_[¹¢?°6*xtg?¼/-ï@Xú?§*؈Ò(?Àjüì,ìü?¦3þÌÛ-?â4ûÕxíÓ?¸í{­›:?×L:E F?·¼0=ý•?±%äm·ÅR?ŸS²ÆL'?é®)GÒ?Àçæ£ãt"?»ÿëþô#?¹"‡eï?¶ŽÊÄX
ã?±çóŽ'–?Ùâz7	?Òøñ1ÊÂ?Ú0"·~ÿ?Òë‡s¸o¯?ÇÚ¥ýs?Áù`¥B€i?æ]Ž¦vw?³5äìij?Ád–ÞådZ?«'žF]¥?Æ-òæ€ÁË?­
0d²(?ÔXÒ:[,?º¾ñ~E?áQŠ!è™B?ÁJÛãߨ?%ÓèäŸ?³Ç2åø›MIXED4FGL J2103.7-1112?ï"µjc)ÀA4Z¬1À9ßñQçSaÀ<hdÓ¿/U@ÍB§šcC?üŽ`¶#=?¼¸KTg?ÝóB¢'åÆ@ @9«ó8@r¤íà˜²¿ç7àìêO¿¡qëCŸ*í¿ËJl_Ϟc¿æs?ã­¿ë¯eŽ$Æ¿ïÿœ}y¨cAGNbcu3FGL J2103.7-11131RXS J210346.8-111335?º©HŽ9>:?¹ƒ*ϛåø?ëÖé¼zLÖ?½eLyÅÁ?š}¦9‰:[?—³Ñ2 ?ÔUOçžà?Èï=3«íÉ?á[6Þt¦+?Éη¡7?Áèíæ^)'?µ¹¯]§Û?ƅޤ™/š?±u!U'^E?è08#X?³…*Jõ?²ÒÀõ±¦?Ÿ\óÒÉ[Á?æ:™¦Q/?ª?d¥G(?Țzâk¼ß?¥'ÉÖtØ?¾©5rAÁ?˜G¢±c?§+Š–~?¡£Ï?¨?í·¯%T?©g#P—;(?šÆ5ó›²g?˜!\q?Ã-ðՕž?ÀÌÕñŽ£?æ;ß
(?È—.q?Ãã~ÏÊ?ºÀ§~ÎUþ?³Fl‹•?¥Í'a?ëŽ×d¼~\?«Ì΄šÊj?°BØO‰k~?ž0ˆŒj¬Ó?Þ4€}òQÊ?²ª±âï+¥?Ó4½p}/o?²å¢S‹õ?Í-"# ý?¨Öª‹äTMIXED4FGL J2103.8-6233?îy–ŸÇ¹›ÀCyÅoÀ8ó¤>aeÀ;éµ³¬@wèºéö?ýº›
7 ?¦¢,+ܨ?»¢é#šŽâ@¯.Ìț@
{H!+ô¦¿Ù/F>¨²;?ðFyŒ¿ß¹õ¤ÝD"¿ßêoŸõÿ ¿åU¦$ÂW(¿àò''sã'AGNbll3FGL J2103.9-6233PMN J2103-6232?ïïf‰e³¨?Tu
˜Kë+?<ɵÿŽÙ?;N>õÌY?Z,:£~r?P\þŽéC?ï‰*xÏt?ŠXÔ,'…(?eÉÆS%1ä?k䬌ðNÁ?ˆBð*úô`?†TܹŠÂ?îÅt¼aè?›§.ú«¨?'ý¿Ö;­Í?"jJK¨Ÿò?•b1‹XÝ>?'¬üDV©?ïói³f¹?wñÝó¦®?zG¾¼Ýü(?^TÄUïp?•o£"Ú?s'˜Mÿ?ïÊr¤"¦?rî<}nž¤?PìûԔÇÄ?Nߕmj?v‹n©›
X?p‰Æ2>ï'?îi¦HóŸ?­²ÝÐd¸»?'7wýpæ=?'ä°¨°·
?¤×½}ºÆ?©Ür|â8K?îtíÕÛê!? n}@/?–—;2Ë¢?–§W(x±?šË
EwZ4?–•]x?Ó?î2ld_ٍ?°ßY·ïU?ˆÖj˜?Ët?s]š™Ú–>?¦£Ÿ†)O?‰&ªÜ˜ÞAGN4FGL J2104.0-3546¿Y<$‰zOÀD´%®æ1ùÀ9Ì "ˆÞ`À<FŸ°4@™ãtÙñ£@ÁDÙMä?³·»B¶³Ü?¡5žPJ?êÈÇ.¥/@ùçb$b¿ÑB°Ž¨¥¿áÊa¸¼¿æċ_Å¿àú,hJl¿èÅ-0º²ï¿ïÿÓ?,» AGNbcu3FGL J2103.9-3546NVSS J210353-354620?ïå²:.ò?lÓ4ôí??ê­[ʓ?Azˆµ#?fPª"¹ús?i9à:ú?ï낷wG'?g2¦Þ_?/íR@[û?ARrÅŞ'?b~wã~†?d0d¸mš?ïºâ#Bœª?r@[ð­°ß?Xòdp?_Ê#e?|‡ÎPêƒ?oö)€? ?ïòµIxný?7œ;'!;?-t2îqµ?;^Ö¬?Vææ\•Æ?5ƒŽŽ"k?ï¾} '?€ž-þB$?TéßMaÄ?Tè•bJËr?{½ÉŒ–õÒ?}«Õ†ÕÏ?ï¿Ásl?"|Ñظ.?;@0ÐMñ?Míî–Õsú?~kxÊC<	?ƒîVgô8ª?ï'HåՏó?›¿¡Þ'?a'åš…‹?_ù!;|ip?‹

$m×ü?|Ö¯;ÑÄ,?ïßgÏG&?W¾"°_v?Cæ:A=Õ?2åê?›Žñ?kç	­áv¾?Tö VmAGN4FGL J2104.3-0212¿îý[Wêw®À>Q2ƒ
À:«§…§WÀ<` ä¶1@!ë_ð«y?ù1†U7	?ÃÉS¯-Õ?¶Îu'ãö?ó£Þ–ù¬@Ògd¾­?ïÒÀÓoS¿î,QA¼
¿›j˜ò|¿¹Ëx1¯·¿Õz«Â»üÆ¿Û쑎2]AGNbll3FGL J2104.2-0211NVSS J210421-021239?ïÁT‹?ž!ç0%?HÜ	IJ?:@‰Dƒ
À?œ~(ü'Ú×?õ	_KÖ?À-W&?'Ä(uTiÞ?ZËLmž.?`£T'µ
Ö?‡<&V=êÀ?€]Oñ—Íá?î'#ä`½/?˜ÜlŠ¿LŒ?Y™§Ýö?FN¼ ·Ÿ"?¦ õ6+Ü?˜æœo6ð?íÿŒåM™ˆ?†më>G¦l?`"/ÓÃé$?EqÅÜǦ?®þî«@vm?†:Ë]*
g?î@µ'å?¤Ç•"¥Û`?\ƒûÂn?S'Ó¬®×ì?«yҞ?¤|65Šë?ï)´âÔ?œÎ+—i†?b5 0<¬Û?l4Ç,ƒÒ?œõÖÀÈZî?›@˜j}Hì?ìD7Q6?¦_P®ª^?cêŒÌdÆ¡?c8J =qØ?»V‡ EDÙ?¦K¨uږ?êr<ký:d?¡¡%0f$?sä-.¯²?gu}\®v?ŗìær»3?¡¤OŸiAAGN4FGL J2104.7+0108?ìªäU條À<ªà¹ÜÀ;®ìÀ<~̕ohn@Kîí3»?þ…ä*·c¯?ԉ݁%?Ìãݵ}Oâ?÷£›0r@µ
$F0f¿ï ŒÒá¹Ä?îsóãqT?Õ%çۛò¿àè`Ļܿç[gà$¿àQþÐUAGNbcuPKS B2102+009?ïî·¾I?TrÇÊd?.õÔcÆ?ñ0Vǟ?^ÏR {Ðý?S
žÞÛͱ?ïÜ6çœº?qÊނy8ó?9;ù1l?EÝmöu,h?pPø…€9¤?o‹ô3#Þù?óS¸þ?†¤¶	''?[]>—å÷?U«mmHO?‹³›KÁ³?€òCgÕo'?Æì?e¨ƒ˜V£?QÎΜh&?7P–úâ??‡­T²?õè?d¢×%VSÜ?ïؘà«ù?gÉԁ˜b4?AÇ¿ÖíÔ?4"7Óñ?qz˜&ßÿ?fÚŒ<Ý?ïŽù¸=H¶?ˆ$t~'?RqÎTy?k»_^ÿÒ?‰óX2ä1W?†%F ûÂ?ï$W?+SڌlÏ?c¬C)ÊMœ?`ÈÿÃäk?™Œ¥òÒ?Œ;nÞ2?ï2)Å-?€Z ÷‹+1?Tìy"EJ?IŠ\›ŸÃù?˜kÿÎ?êRÁ.c4AGN4FGL J2105.2-5143?â÷«ŸDm1ÀD¹Â.äÀ;.á"ÚîÀ<‰"'Þº@yÝîÞ¦@E¦'¶(F?ŤK¹¼Ïª?më«¿säL?ª%vkí@ô¶ùPäI¿à|¿n?x¼¿èr@úœñ¿å­A—$¿ç™¯Ôn¾¿ÚQ¯<Ü)¿âÚÒê?¬AGNbcuPMN J2105-5145?ïÚò|‰¾?p!¯¹©Ìó?9'Ž«q?+}Jæˆ?qg– ÅÇ?ofƒ\ãP2?ïʑû"_?sÞ"J°ºâ?DŒO+Ó±?NR=Vô5ñ?x%x@ø¨|?qt{¥,gÅ?ïW?®pc?@úkcf?`ÎB«é®?H(ú7"_?"@ßy?~w0㠗p?ïØÇÎ'"?Oð"ã!?0ÁkÔóí??…+U¹i?r÷T5?O6ä̓Ü?ï'9^y¿?‡°d¼?K!CÀՕ¢?>_`.u™?‰ÿ"2B¦?†˜³hîC$?ïb"º?$â¿P®?TdŽœ{ÑQ?f+550Z?'xD§}F£?ŒqAVy˜Ï?î¬ë?†É?;§ƒ¹žÍ?k!wÄèí?`	¦‡•?£4–8_?ŽcûÍÍE?ïƒEþ£Ü?qª]ûu?GöÃÈ¡^²?=e™?¾þ?¯pÓ?qig+Ä
:AGN4FGL J2107.6-4148¿µZ Ù€™«ÀE>$_ZÙjÀ:'
[2U¾À<|2;¼n±@N ?ûîx@Êi`êM?Å–)̓×?»¸€ºz¾?ópnAüú'?þ0«#uü¿ÏkõÇl房à/ž˜\¿äo¾Sã,¿å`ºÀZ΃¿ê²M?Mó©¿ïÿ&ñÜPÎAGNbcuPMN J2107-4145?ï$Btä?‹àÑâ?dú]—ËdH?RToÃ-N?˜ØsË´ò?Š å $Å?ï_˜ó¯?Ž?Ls)?lÒË
ø#	?k_¬~Ö¬?r£!ÿ±?‰öÙÕb·I?ïFÕ|ó"?ƒ³n÷Ãg<?sڟy$ª"?te_¼d[?'.· Dù?í)†®è?îí†òDx?s'¼£'lˆ?‹|³Û?]^?™—Ç睤?p¶²WvK›?íÝetµä? 
âÆÓm?z²iw?i$ZðÁê‹?®ç'iSñ?žÏGa¤›ç?îX/Œ4¬/?¢°‰üÞÕ?~Ïò]ºH?'Ùs¦LNÈ?¦£èÆÈ? ëH›¡È?î´>.R¾?HÀîZ,?ëXmCö?~K¯	§ {? C•þoâ/?Šw¹PíN?íOV·><ž?éHÿ.f?"̬׿
)?z§D܌¶?°R°dF?Œv*R8;AGN4FGL J2107.9+6006¿ä(Yã÷@ ØÀßXÀ‹À9î²-å™À;'KZqež@"eæ
æ@ß8úóPÅ?Ë$kYÀ:Ã?ÒS:»@gæ³þŸ®?ú˜€â¾{¦?çôS>kuš¿ÑDŒÂÂ#¿é´÷!¿æ_iQÓ1k¿ï÷äÞ;Š¿ìue<š»AGNbcu4C +59.33?á"N*Pg?Ã¾g·þ?ŸPB¢6Ø!?¢ISÝ­?Úâ_€Ä
±?±µyôã—?Ø¿—¬ÑÒ?È׆ú…—¯?ΙXt=ó?¿\µQtօ?×ó¼")?Ä
\M?â`H5›d?²¥·Tjm?³òBô·Ù?žU>ƒšë?ÖBß
A1#?±@°9è0?ÖëïuKå?¡RþÈ¥ÿ6?ÒW{"D?¢jnÂW2T?Ö¼"÷¯Š®?¡}—D$©?ÑM§9O?¾ß™m¤É#?«Þ¸Í/€ô?¢ÇüÂ'Y?囊±©¹?ÀȨÍ?ŀúqÒÙ?Ä"E¶SË?×Ö8ä֌r?ÇßÕÈÉÝÚ?ÝiI♊"?ÈÚ¼ƒ1+?×WÅ¢Ä6?°Éíâœ?¿÷k"Ä9ù?¤‰Tê½O?àU/¼}–¦?²+ bš+?¾Ô)H´àÙ?•èfûÜ?ڑ
þ¥{¿?¯_¤Ä.¾e?ݹê¯-L?¬ÑÙ@Âu­MIXED4FGL J2108.0+3655?ê጖'/ÀÍ
Œ°}À:ÊÓÎHÎÀ<&¿»lR9@ x¿úeñ?üe&*64o?Á?öût€?ÃΕ¤Âl¢@ª‹ÄÄÀ@̝–~\&?éåïé1‡b¿æóóiâr¿Úª|€Y+À¿Û
ü]^*¿×Ù#"™Þ¿ëS9bøÝAGNbll3FGL J2108.0+3654TXS 2106+367?î
®X²7?¡OóZƙ.?yvøüH@?ƒb"+ï¸?¬&J4µ
?Ÿú£¤ÔC
?éºÁ0{6Ç?»»U3Á¬?p­ã)–]?xYo•¶¡l?ȏŒ&¶Åq?ºæÎÚÝËg?îL —©+?¨SG…µ?u®Á5Í;ç?joUùˆÎå?¨€]äÙ?Ž7Òo ?í›"ßíª­?ƒˆi%Ÿ€?'<ThÏ?_ã²ë
o?°äv~ŠÀ?ƒ-5'½î?êòëM'?¶Y¶çžl?™°]RÕ?© Z}ú×¢?ÀþG Ùqÿ?²1S'>Հ?â6Bwìm?Æy‹"ÁÐ?~{pÍ<E@?"ü'ôO@Ý?ÛŽ;Âxá?ÆVç|jM•?êê*õ»È1?¦Í¤5"?è*œéª?ƒ–戆1?Âxр™K?¥SÆKŠ_B?éܸ۱ʛ?œ¡ÏÃÙ%y?"DŠ.?~z>z±y?Æš
ݹ.?œ|ü$à&tAGN4FGL J2108.2-2454¿ïdÊÝªÀD¼j~ùÛÀ9î/²u2²À<Sîe£ÈÈ@³P–‰@_êÄ.˜š?¸œ£å"5?§¯ýˆ¬a?ê¨Ñz±w@q¢Æi}¿Ù#ñÁùµ
¿ãô~ø-£§¿å¯Z@hOö¿ép'D¿é0aœ¨¿ïÿì^ãe@AGNbcuAT20G J210812-245233?ïõÈíLҟ?F­ñm/×?0¥Š@ÚN?%	;ÁF{?PDÃ(šÍ¹?B×±Ð
ìl?ï×Vo²'?'x²‡fè?9~6OŠ1‹?E¡i…ÄŒš?r¼äúüm?¤y@»‹w?ïµ\¹ûu?kœ0uMú?VP$Ç;ê?D¸&Pí?ÐNØÇT,?jŠ‡²®>õ?ïÝé1˜?Pá·}Í»«?HêØ?/Éۑv?l¯è$rú?M¨7÷	À9?ïäNÎð¢?`iWÀN?BъŠ†€¾?7Ü´ÂHB?füΡ¨ü¢?\'S,·hî?ï€Ë&¯l??BI}VÕÀ?LY%Š®Å?Zï"MV`?Ž£ûVÔÌ?^!†Sò?ïn"sJ?~‹Ì¹˜óÅ?e%•¶—?c{ÅÔ=`?õñÅeá?{°Ìëppê?ï¡÷êÃê?qçQzŸm?aå:»•}b?QI	íí>i?ƒA³I["A?m8Šb&AGN4FGL J2108.3-4824?ánÉ_ŸÀE)Ëeè'À:ÈV%¦'¶À<P–ÔÃ;T@æÅÎ*ñ@B÷<@?ÉÔMI´ÔÞ?'4ëïý©?ÃÏÖ¢"@QRÔäv¿®pXœhß¿åF/ßÁœ¿è58@¹-´¿êÎô$)ªô¿æ§­ŽC$B¿ï]6=©¯AGNbcu3FGL J2107.7-4822PMN J2107-4827?ïëfÞäÚé?_©ïcè¤?@HS?=þÂ{q*?`—[Iÿ\Õ?\<MjÄR?ï´ÓÍ®/d?~2ÛØ*?R?•1wÄ?]»]ß
R?€ƒãöpõ?y¨ãNDŒÇ?ïÖ'·?‹fåš×Ò?jÔæC7Û?itÅ°N>?™+€·ƒ6?Š\Š¦	?ï¼"üÀk§?^<A‡.g?P®Yé")L?7%^«¡3?}ÂëDUž.?[ÌI'¼á‹?ïڌƒå?nã4?'/?OT##UÑ?JD‰ÌÐÊ?mžv¯&!<?k|qFêw9?ï1Á–bØg?™7©ûj?còmo•÷:?vcº¸<m?—I€Ù5?•ñJ -ɜ?î)–/	‹?›ézüw??|çŽÙôëá?xë1%ä®?«0t¾£&Q?™íÆHwˆ»?ï=JöjÍK?|mU!©K?f­xIÇX?T˜¿ÿ/Ý«?•€ý¿©Â?z}½,µ,€AGN4FGL J2108.5+1434?è¶áèV¯ÔÀ5¾p'IÀ9¿%ª´tÀ<#M"M@tN?þó'@"9¦û`?»ÿüOq ?Æ #÷V
@@ç6žË@žâ¾ü?°‰c–}Zt¿ç‡ª^7éɵ ÝD¿èûDå^³¿ïþgä맃¿ïna'·'AGNfsrqOX 110?ïñʪ€-?Qâkšs¡?Kk¥"—Þ?Aê´Z5c¹?Mi°K£s¸?H0ªíÞ­æ?ïÌäè«U?z-QùC6¯?TyÁ`ª´"?b"Bâ^¬?top¸'?tBû¾¥K?ï«ßÒì"?uhòh*÷Q?cXJ°>ò?_¡i¹Ûm?€1ø¶5·Â?rì»SJyO?ﲔ|Ï3"?]÷µD¨?lNÚ?P˜'⛸Ò?xŽT€° ?U=•¬¸üÕ?ïä#	ç¬Ä?`"ûýdä?`7‡€c<?V0;M³8
?WJ݃²1U?Ošï]¹×ú?ï_Åö*$?"çÎß5U?npˆ—«eD?{«:ö]?O61þÄ?áÑo2Ž?ï_ðh]a…?†ú]ãc|?r̒]ò?q·i E"à?Žø׋¥aº?"U±tAu?ײַ
x?€ÁÂ/Íg?†¥jAÄê?sÐĬx?'·
}?uë‹çšÓAGN4FGL J2108.7-0250¿îì@Q÷À?–E"}À:Id?D¹mÀ<cÿå(
e@<*žµ@z͹[ÖÀ?·˜SH|p"¿•4beÙVQ?ÞùI,™»þ@ƒàṗ?îñ/'¤ŠŽ¿ß'r¡L%¿á´M¯¶;'¿á§UCÿ3Q¿ã61µ"±«¿Û×[µ2AGNbll3FGL J2108.6-0250TXS 2106-030?ïɹ	Ôó•?j/¼èr'?K¡®œü­?:Õs·y\?w¯EHx°'?hB€'‹‡K?ÒNl?ƒÈ¹bÑÍ8?XÏó~ˆ?[_ƒÌ:o)?† 'ë¬@M?'0±Xg1?ïoFƒêR;?y¼gô3Û?f B֗cx?eÜNÑ?Ž¦N@§Pl?v\û×Ê?îíɚúRþ?vzx©£i´?sdí
T?RJÿåIb?mÆÝ¢ì?uS"žPl8?ï†ò®Äà+?}zr'¼¬(?a^Ôõ+åÞ?R/žÞa?‰ëžÿG?zoI¥ï ?îÊ0×›ˆ?¡ÛÇ÷±ð?e"´.?3j?o0c'G*)?¢§Kâ@L?¡™@>"Ó?îôÖÑ)ö?†`ùƒÓÎc?rQ|Ä&®?k‡hF<Þ®?œÐƪ¿sØ?"ƒ‡O
[?í¹ƒ€
é?'Q*jâ?‰ïmV\½w?qoÜe'îM?´"F:}Ӌ?'‡#Vc'`AGN4FGL J2108.9-6638?æUÙXvcµÀCÄÑ¢À9‹á¸À<YŒ~þä@‡Ëz½5€@ãÔk&¿‡?«£cUdá?yž	>7á'?Ωu¯¯†@38üö¶*?éÅëÒK'Ï¿áS
æû¿äÚ?çvœ?¿Ü!¾@ÂèÈ¿âÂâ2ŸE¿äÎ%\°ÚÿAGNbll3FGL J2109.1-6638PKS 2104-668?ïP•i^=x?¹X (·Þ?dàás¤DÊ?‰­s|_³*?"Q6¥ïÃf?¶SgN_s?ï¸ÞI旾?(6+–?RòV'X?_ü[TŸ	?~ÔY~	'í?yþTinŏ?î	ó½ì#? \ ÅÖæ?uÏy^=ˆ"?|]¼BîÁ"?¬¦Ôö©úl? …]™Û€?ï‰TÓýÿ±?iQ,;FûÜ?s(Ĩ¼¦R?UX¼›&º?"h·xv?båj•,œö?îjÌK6xý?¸Ù\1—W?zE=ØmáÐ?¼;kL:|?¦
"í~?µfõ äí?ï5óˆ?ï?–SŸ"yW?_…œÅœ¤Š?l'
d½ƒÖ?—IB"­ûÜ?"ëŸþÛý?ìµS1çií?©'izr*ø?zB#WEPµ?|4ër6Ï?¸±D<7AI?©XQÎw!?î箓·éw?ƒ­<Cg/Ò?ˆ3qtöòÇ?ry²á±d?–ðtÓ®Á´?|{‹M8àwAGN4FGL J2109.6+0440¿À:¡^ˆ³À;䃧 À:f̧ãß8À<-Q{×@ЕYC@ÖÎãþAº?³ˆX(¶?žÚ܍"?ßÌ¿`Ón?ÿ`™56Ä?îÂL ˜?àöÚhµÌ¿æR,¾}¿à+›>µGu¿à¢–˜]Yw¿ïüàÎï½AGNbll3FGL J2110.0+0442GALEXASC J210940.09+044000.8?ï'[<øÀ?uÂ?VâL×?X'¦zºp©?EèÎv»¤œ?ˆ¨´d''æ?tXkõœ!Ó?²dl?u}K€j?Zˆ±±¿³e?XÔ[zçµ?…À¤ß?{»9&ê1?ï(.Ä}aÄ?†ƒ¤¢§®\?sbùÜ9Ñ,?pþ|¡Ä?–!hü&?'9/O¨f?îBö=Ÿ?€è:Gî»é?…Ú5`Í?fÝ"(lØ?¦™Z
tÑ?~'cýn–?~}üR?vK·±?pŽ6OŠx?b¯µšëg?›$¾›ô¢0?‹­¢j?îÝ5" ¼8?˜
iH? .?oùŸhcŠJ?sT"°ÈÏ? -èÍÛ×?–
:GwÙm?î¼;§md?™¸²ÿë3õ?'è—yc+?|j¢¬ƒÿ?©º8]…v?–ª!Áye?뱌Ë2¡q?˜|˜ýžn?švK7–,B?'_¬P¾þë?»ÖØó\ë?•27Ëù\0AGN4FGL J2109.8-8618?»i¡óôó¡À=.î¢
À:ˆ^iAâùÀ<pär@!™lä.é"?ûdÏÝùDû?À÷g€æ¡?¥þ®Ç(H?æÿ'ö֌?ýltóG
?ílŸWŸ¿á}Ó %¤Õ¿á•,b³®¿Øp¤ý[¿È	û÷ݝ¿ß IaûcAGNbcu3FGL J2108.6-86192MASS J21101113-8618473?ïžA•\Ú2?'Ê:»¶M?H.ÃÏü7?:Ú¸»À?†ì¸¶¦€ï?'k>;sÏS?ï'ñ/"Ò–?"Háé'ö?_ÅQuîå–?fg=
§ˆ?‡K	݇+Ä?€•Ã
û‰?ï/¯\=\q?†›ãê®?c|ÕT
V?e˜–¸c?—šyϊþ\?…‰n>§#©?îèËþ=*?ˆ}tù?r~?á˜g?X´"XI*1?¬«GB¾ÿ?ˆatk
/Ç?ï6¸6Eiõ? ê.¨!+?^…Á´ .?SVt#½ó4?—@ÌXe?øð ¡Ñ›?îÞr¾°Ì³?™ÒOÒÝ$?m
úÒë%?sÖ}/j£¥? H$hâd?—ärÁúœû?î(ªèË1?›yÚ¢{Õ?h<>"ÏË?b&†¶—É?«ñ›etð?›AÇ[ÚØd?ê‹$¬Ií?¢ÛJ¯tÎé?‡9ŒÎû?wŸ|ps?Ä_ԍÃ?£N¼µ?¢AGN4FGL J2110.2-1021c¿Ø¶¨s&=ÀA½¾ôœõoÀ:¢v0íÀ<@õ0™%@t››&Œ‡@°HàC¢?Ëç"Ï/~?Å.¾¯R¾?ð…£dôv@ZKë»ÐP?ë™H`–Üx¦ojñæ¿æÌ<6çô¿ìŸÂÞ6œ¿ïôÁ]'çü?ïÐù^#øAGNfsrq3FGL J2110.3-1013PKS 2107-105$?ïxƒ§ó?"œ†\´?eªÂÀ6?Yû;š"Ò?ŠÔñc£÷?ƒ{ÿŸnÛ?ïP¬u
æZ?'Ofg	›Ø?q¿¢f¢™n?y…Ç⥤±?'zˆ¼ƒd?Œ{±áw?ïÌF·kß?‰²,lØ`ù?zˆ¦Ã}â'?ugNzÚº=?˜DM}Zuw?†¬¹fP‡{?ïuuU #?{…-?êÙ?sSM‹uRá?WdF±K&?š}íŸ2é?x偐?©?îyß[?¢Ÿµ,;*?x›ŠK§*?rŽÀ"rž?¥N™WÅí?¡òx Ø|?î '"i?¨…,¦Ü`.?ƒømš!PË?'iîO6E£?¨ÿl|Æ?¢}99".«?íûèÖ?—ŠU'38¡?‰?…ï?ò?€y®½!D?©ñ'¿à?"Æ®#W¬?ìòÊxgMu?œÿr?ˆ¬|ùs\?wgÑÏ+Óï?µTž™n?™;xM¯æAGN4FGL J2110.3+0808¿ "$ÐôîÀ9ëOÆðéÀ9ÌŤº_À<6ڇ s@Ò¡ÍðŽH@ÓÒåëÄ?¸r¹ÛÙZ$?²)°þe @?÷™DrØ@{Çb¦ÿ?ï1ž2°¿ä‹a'¦ãÚ¿å$†È½¯¿ânå€ÍÅÆ¿íKòa±ËÀ¿ÔOG› AGNfsrq3FGL J2110.0+0812PMN J2110+0810?ïëîEöâÓ?S.PéÞÊ?7ú«›?'¬h•ÕÆw?a0èú+?Q¦ŸhDõÄ?ïè8'Óé?iÈuƒ_ÿ?4j¸­>µë?Bþmºê"?e:T
¾R?fŸ"»Ýäg?ï¹k¬A"?u't"]¥?[þ2_¨Ð?^‡Òx¡D?|J«ŸÖt–?s|èê2g?ïÛn¥œ~ž?L;þRµã?FXÞwÓ««?(Ù"r¹Ÿ?nû"Í?Iñ`­?ïÜԘâÔ:?a7&%KÚ?F­¬m$?6ŽGB*ñ?m€­ï?_Pr.~ ?ïµï¡@µ…?ƒ4dßÁó?GÚÒ¼áÒ?\;?Šô)!?jtj?wÙ9DÄ?ïŠCt#?€HuLK'?kGFÄj<²?r[³¦©V?†§Ýšž~?zžÄښª¹?›Ãö?lvµß~4?` 
‹ºy?I)<ïßs[?…jSRÝØ?i}j?‹AGN4FGL J2110.3+0404¿á=$Dœ«âÀ<@vžÂÎFÀ:œiW²n}À<T§i¦@  捓&
@>:}ªOÊ?È÷·1/"?¦FŒ~Õô?á6:Ÿ8?@©m˵u˜?ïî5!õÉ¿éV­@•ql¿à֋\¿ôw¿â:s™TÐ<¿×àcØl"¿é*''¥AGNbcu1FGL J2110.6+0403NVSS J211019+040418?ï_D—šÍ?8Î`rFô?Fo"ª7ÿ¹?5ÌFË (?"cóðR8?D^åϹ?ï­¢Vë¡?|ȯPvû3?RT©d7Ä?V8ðlª?'T¿ãðÖÈ?y®'ì-½Œ?ïK³Óò?ƒâÕVlöß?[»ƒ/¿;?USIOÀŒÁ?"ÍæìøU+?ƒOæÀï—?ï+âô3ø?t)Ÿ>©Èä?S¼ê-ð?7Ç"n†—?™Gþ1ÎÎ?tãŠ¸'?î]"&
ö? ¦ö˜Zü¼?]
èÀ…+"?RKþžê†?©>^VïÈG? v®xÕ?ï*ù 6ä?'~ðöͧ=?\S£Cþ
ã?exØöP%?˜Û'ÇÏH8?'|¯mN4?î/ƒXd›
?˜+sGá›/?fÅ)ŠPó?]E|•3¤¹?«›wåʧ?—Ö؄ßúÜ?íj¯"Öáú?'¬vp=¸?hÄÂã ?W渜™GG?³ä_h)æØ?'Ê
ÞBž"AGN4FGL J2112.7+0819¿á{ƒ<³jÀ:O9_JÀ9ìT3]û^À<%aþÈÈ@ 'òK—
?ü˜˜è™²?ÀüššËrÛ?Áƒœ—¥Î†@X¡ß¹8›@
,íZ`ô?±'l©¡y¿Ë¿ˆ®å±¿æi\ÜJ¿É ¹¿ú¿Ýù"ÏbÔ¿èîö«¢AGNbll3FGL J2112.7+08191RXS J211242.5+081831?ïùÃ=š?72=íV?&'±4eÄ?&à,Í8u?FFÐdKB8?3ÕÅ03sÝ?ïØ&.ŠNo?|ÂÍåd"ó??mÕp?INc¥a<?qû—Ó(V?zT'pÔI?ï«´ÚpW	?{Kk¡Ù@
?SXÑÛÝê_?OôÌiQ\§?'§¯2
h{?z³"¥q.?ï]¶¢Ê?q†Ý»Å?ej§uU9?G8´ß"Oö?›Fô[1)?p"ØwÃ`ˆ?ïòf"Z=?H'E‹!¨ñ?@¢èȯ?8#!H
²?Râºß_Wœ?A7L×Uºð?ïŠl'+¶4?‹'{èٝÁ?RœËOæœ~?`&ÂS ŠK?‹F	µÇ‰?‰þÓñ^p†?ïråü·?ƒo€И"?_×è—(?c±?êÜñH?Šf@"Óc?'ZG˜?팎«ÿÍ«?,èáîV'?{
­Œp‰Q?f&ƒ_	?±ê¯ÈXi'?Œe´ý²¤¬AGN4FGL J2114.7+3130¿ëKˆ™c‹7À'ÄÂÖ©ÅaÀ9ïÉ¿Ò‡À<œšÕÚ@›`Ú5k@(Ç\Jƒ²?¾Œó$?¹&äàÎU?ú:bÒ]0@6~jê¿¿è÷›bFœ¿Ú¢^¤¦#¿äŽ	Bžá¿ßë‹Ô´ø›¿í.Œ¥•P_¿×®à}®¬AGNbcu3FGL J2114.7+3130B2 2112+31?í—×Ò[ÏV?¦‹9
ŸÄ?bü=•ß?rüU?±K¨øEò?¥LÄ]l·?ïˆ&yD?Œ"z+üCn?dݼG':~?p'àýƒ;p?ˆÈG_˜Ÿ|?ˆri'ځ˜?î8Ü3¶Õƒ?˜›BzÉ«Í?'!sà"?Š;D?C9?£á}CX·€?'×G ¼=Q?î´Ý42Y?xesq»ª?ÿrï'EÒ?`Åv¥ücö? 2JPÂK{?t»MðJ®?êœV¡ÐÂ?¹«!+sÌ+?•'0·ªg?‰‡âü¨ÌV?ÂÞe ´ê?¸£ʙo<?î'Uå墇?§wœ'Éü?Ò«ûÈ@'?ŒŽ¬Ke°?¢àL"ƾ?¤¼P–°?ëË´¦æ3P?¦Èü=ë­j?¡ö–dÖ¥?•×Ս'Yœ?¸§R}.¬?¢e"œ÷—Þ?ì‹;Ê}ßv?—â¬.²ö?˜Iï´Är?'KEñJ^?µ"¥¿MÐq?"ƒ;¶èAGN4FGL J2114.8+2831?î!£ö¿èÀ+ϑ`4PÀ:-qRR³À;ØÔà—…@H'1·]@[˜fÙS?ÅóyÄ<0?¿Xòà\̊?öl¡«¶Ó@€?ƒ"´¶¿á·ü€Ä‹‹¿èú~¶¿D¿è•«}Ç«ü¿åtÞÏ-пïþÑÌæÎ?îU—¬Y¾AGNfsrqB2 2112+28B?ïù÷'¶:(??j'{›ß?$.
{w`Ë?Òŵ`7?C6°8À?<xüQùL?ïΙyŸdp?}©6ÇF¹?KL»`»ñü?XiÜ­?uI«ÈUѼ?z/;¶"Æ?ïj§¸¸!?ƒÅ©íõr?p0Ṍù—?s¹ã÷âŸ?=¦åäì?€ªTæpä?ï¹	áL­û?d­p—ëå?LÊ°1ä?7'\v¾w ?á¹{[Êè?b£T½i…?ïöÛuËÎ?Kbéˆn±p?3I/j¡s?1«_«EJ5?NGú#ÔQ?FÀùQ\‹i?ïâµ0<Í?'/(¹o?a8!(7–?t)5}@?²?‹9Jyuâ°?, '9k6?îçº;O·?'ã¾Uæ?{j5¡J/?}و¶9‹?œTî/M>…?k<Eî?ï
¤^LD/?…=ÂÞUn?i_s·>'|?[²Véª?›…»Èù?ƒÆÙkµ;|AGN4FGL J2114.8+2026?îɧëZÆ9À39"úÖËSÀ;
º(…ZGÀ<zÙ@x–@ wÅ3{X@qæ¤å'7?ÍĊÉr$`?§ë#$iî?Ýð¥dSÉ@	EíãðQ?ïÿàŠï²«¿éC_›q
.¿áÅÛAÖ¿áí6ß»¿ØV}JK¿ðAGNagnTXS 2112+202?ïÏ¿Îa¢\?€Á:?"?&ñ•v)Õ?*o³œC$ê?whŒ^©i?€'g1À'?ïÒ¡êdÒ?tÁk÷'É?A³\"¿—`?Jbuçÿ³%?txŸ`ôZ²?sEø‹Û(¥?î`šmÇ"?Ÿá2Ÿ	|?VIŽà÷/Ü?c·C«?©D¸3Þ`?Ÿ¡´iI@?ïµLc€?a—€â€ú¥?:žLH›,?!@]_e\?×ö+aá?aTÆÆ@s:?ï›Lló§?‹%X"W£?4õ`ÛñÂ/?4®¨ønÖ?ˆ•Ò•ž?ŠÈP-˜SC?ï†-!‡uf?'õ`wK°?Sm†Âܛè?gCBd€=?Œ̦Jþ?ÆùW6¡?ígÜ6ú}?¦šHµ]?ZpÁ/µ?cÀêLÙ²A?´W[Gk§Ø?¦}Zßú›?ï#¥¡²?×PÓ9õÛ?OÍ-åPY?@uð&¬Õ?œ!êY§F?ÓäÉ6ÍïAGN4FGL J2115.2+1218?ïhQúi#À8k•¢"À:B—Ò<èÀ<S‰®j7@ "¸ÌdÈ@B¡e?õ¹?·DʊRS࿘=~e¶"%?â5e<š»@w°˜¹ŸÉ¿Û9"5‰û¿ÙÏ~"DÎf¿æü€xá=¿ÏÔ<ãÚÛ¿èmH7§6:?ÏéÊÉàAGNbll3FGL J2115.2+1215NVSS J211522+121802?ïñ¢4¿?O5éå¡ã§?0¡'"ðÇ?&˜wHQSh?X"·_VÂy?KÀXZžá§?ïæÇ¡Р?hâ#²Ÿív?1°©Á™ŸT?A‹a$Œ—?g(-®~?eÖ×K+¦?ï«Wº&,?vìT%•ì‰?T:úËåQ?[îø»OU?'§
êó¦?ubní?ïÁŸ…@ò?[ítÈ3ø?M¾IÏÚí_?3¦DlËØ?{Àfî鰝?Y©ã¥îœï?ïßÿ›šêk?aò
sG\¢?D;ΜÉ ?<SÑP?jñpü£«?`Bäc'Ôº?ﶵ˜A™—?'«QIk%?B‹@ö»?TÍÏ4êÆ?*+	SF?€ÙÇýõ)³?ïc;má§G?ƒÈÅïÌv?`÷úϞÌ$?bûH¯ ð?'y'ñ'\—?Ÿ-ÝQâó?ïI­uÄ}H?xcêtvI0?fšgˆ¼?U­¯w
¿ç?"÷S­ÄL?vðP0,AGN4FGL J2115.4+2932?Öö"<vdÀ*¤$=Ìê)À89'T؟iÀ;u™ô2ld@î;'Ó+â@òŸYÌúð? ¼nþøå?»¤Ùh¼ü@Øú†C@Ѫc@l,?ïúû^Z©D¿ÞR%fÁÕù¿å7àAׁ¿ãùê<I\j¿éJߢ<€d¿î´ ~$É
AGNfsrq3FGL J2115.4+2933B2 2113+29?ï¼¼J[·?rc
ð€§v?T}̉?NÉB…ÐA@?|'—!¬¼y?pT¢ÀÉ?ïØý3ê4´?€ÙýT"‡©?E¢÷'Û-¥?XRц·i	?pÍ6({·?€	¥w
‹?ïRHÑü?'ª_	†Ù§?zЂֵâ?'8ªªY·?Ž¬V¿è(?Œz[@–‰?ïσԌ?\k0Üàûâ?S0b·Çå?@J¬û
?s¯‰ú?X=¼¯	w?Ä
?{=­aVïì?ZÀ¡m:ýj?S>dL*Z?†¡;!Kß?xí3 Ë?ï¥j#E"?'¶1¤G?^¬k±fƒY?®£î?'Ïé´§x"?2q[%ÚI?ï-ñªÒ§?–ÅRãk?'!æ¶)0Ÿ?‡J·jW:8?–	Nn‰0Ò?'¹cZå¡&?ï€%ŸÅá?x¥,őâD?jADâÀт?Y÷9+˂ñ?‰fnVÇMa?uŽ·Dý™tAGN4FGL J2115.6-4938¿î¯N-4—ÀE®6Á]-À:­Y-˜¿À<œ™µHKÉ@.­f*+x?ÿPpûëžI?Æ<,9
ä?¶X|ÀÞ?ñZë­ó?÷<T "ž¿ß¶,A§j=¿çûš«'"¿Üˆ%=|7^¿Ý:ŽÜ§5d¿â\LœÄß¿è òž˜†õAGNbcuMRSS 235-024179?ï®xÕ"?x-½Épj?@›u˜±²Ø?6=<ä¾m?ƒrjr8þa?w›ÆMŒdÐ?ïo`ºŽv?‰÷¨¢ÞØ6?g_Føe™?i§MõËÛv?ŽP-W
¯°?…s¹Õ(Ï?ïp1^zgX?}NwAâñÐ?cDùø]®	?^Õ³ê›?"iótèp?{öYqŒ
ƒ?î;h¤ŒÅS?ƒÄÁ×ûzò?|«ûÎorª?`T|ðõ®?¨³ö@}bp?'¬9™¨¬ã?ïb¹ôâ?†"ǐ¬?PÓ¢Áðח?D°-&é?'›‡Nv,C?†lìÉ_?îuã*¡2?¢Z	Š
!¶?xãÞo6à?Q0½ɚ?¥…Qˆê¼û? ~£"s6G?ïÔ`"ë4?Š*>;%Ð1?oªðŠëK«?nÓbÔ3?›°×¹­?ˆ+ |=¼o?ë]쏊Ìø? #ÀÞÞÆj?ŽþɌ5õ?y
QIÂ}?À˜a(lŽQ?Ÿ
½5d—­AGN4FGL J2115.8+6753¿ÞæY!³Ò@*	"ãÿïÀ;Dœ)¥ìÀ<"!É~c³@!m£4"‰?õÒ¼›&b?×u»Cš?ãӕsš+@ryJ@;íÞrÔ?àcƒ'«ìX¿ïÒ5A€R÷?áóRÝóe¾?ïÅèít¿ç&~"j]l¿Ýqü¼Ô‡+AGNbcuNVSS J211618+675324?ï‹E²«}6?®6"ç5®¹?yg#
jކ?®úšz?€{Ƅ)_?T0 ³§?íeLÂÈ´\?»*ÕÎuÈ?²ÕÛBÞ? ÕÔ!Aÿ?±?GG?·k•BŽ?í¨£ê¼? ÍV&×?'émÒ[L?ƒR˜j,2?°b²Pði|?Ÿ~Û#èí‰?í@ZxŠ?¢‹oR{Ön?)ÕëÊ2ý?x†Iá)ä?³×ñ€ŽÅP?¢5 hî:?ï:Œ–%ñ¬?"ì…€±6?€hè^è?†ÐݬËé?¬8Î?Íý?Ž1<«/ƒ?êÔ·ÅS±®?ÇS«^~Þ?ŸyïìGͅ?¬áÎfˆì?À½âí(?˜?čjìÝäL?ëõì¤63K?¨ÇY…ØF©?Š9µ6
܆?ˆ"❋Å?½	d5gH—?§Á³?NP?éj2ýiˆì?¹èÔC¨e(?™êŽ×à?¢[ܘÉo]?ÇÛº6®N?ºZO½OAGN4FGL J2115.9-0113?ï¦Ç¢kzLÀ@'¼ÓZ…ˆÀ:M´ÒÛÇÀ<d•^¡v@Ng¹L½H?ÿùäwä=,?‡o vØy?ÀOâ€é'?û°ÔéÑÀR@šsPڎ¿ç*SÆP±É¿Ý‰å£©¿àâçÁDÙN¿ÜxwÀ«×4¿ïŒ~"ƒÕã?é³>¡%AGNbllNVSS J211603-010828?ýòM?­k·<¥tZ?\žºøZ`q?qNR£Üؤ?‡¾i)0ÈA?«WùCÖÍ	?ÔÝ´É?…;óqÖ?`xëñϔi?mÅ{Ü?"8O¿ÀP¼?6íݐ'?î♃°_j?'I¶I¬'?ˆ€{5a}ø?†ìd±tE'?—l'êéË?Š|üÆ»?ït"yã¤?pôY?iÕéé)°?QuˆXÓ#?Œia¤|úç?kXq^«?ïjÛs-Ê?'Lç$MX?qŀñì?w}cªŠ²À?Œfb¸ñs?Š×…d7Êã?îÂsözxË?¢Ÿ'G"ý?s?P!?/(ìÆ,ï?¡Zîéü4N?œTn	?îò0¾º?š&C¯®ä?'ÿ+ۄ?% j'Ñ?¥ÁI …[Ÿ?"#9œØ,?=(Í?‰uþûAV?~FÀ!yh?k»µLLd«?£Úìõ1&?†Ž–¡»¨ÂAGN4FGL J2116.2+3339¿Ò~5_ª­À%MOçžàÀ82LOcëbÀ;[í¤³©@¡Üí+g?ûòˆ-`‹[?¡Sʂo±i?¹.nRn÷@]Û	íÀ@¸Ü&$?æÇ·ÿá!C¿Ò½·†ªØ¿Ù"¾h…û¿ÙšÛ
,c¿âQßƤ•¿à`䡪µ AGNbll3FGL J2116.1+3339B2 2114+33?ï³Â;h$Æ?¢¸Mî-AB?J×D?ƒD"?FŸ"9!¦¬?aüð¼ C?¢·I>®"?ï¶RJá¶Ð?‰®'K²á?JkmV°"ï?V|—·ãwÜ?€Ä¶¼²?ˆâS)šC"?ï‹cnlø¯?‰ñuQYÈ?s8Lüø®'?ë¬pÏ?ƒŠýà0é?§~£
éã?îño¹¡Kë?€)‹ËzÒ?iaÚ¯qCÐ?Oâä¾*íã?ž¥Ín-;??~Çpµrn?ïÂv…uþ½?vЮ²É)?BMœ˜þ]¿?;£:çÔÌ?|{	ÃC¨I?v%i¼Ÿ<£?ïHóÔ"? Â±DIõ±?böèâԌd?|]‡íb*?"'Àh_
?Ÿˆ1?Ò£²?ïuè¹Î?ŒGlïû!µ?rĉ…C"?šcW¥?‰UÁšËÊ?‡ð¨G}?í¼rÙU5*?"ø•†9`?xžÛ
´sè?b¶qªàéb?°'{…®ìl?"§M˜V{÷AGN4FGL J2116.3+1015¿ÏÌIôYoÀ9Ý˼+"ÙÀ:û,¨Õv¿À<e¯¶;Ð@ÇXÛch…?ðx
Oš?Ü¥0úØ#?ïÿì´É È@®-±éò@ƽñÿÁ·ù«
	¿ê
aw¤Q¿Õ©úºÆ»¿ëtÙé¿ïôL¾´ ?àV"Zî¹AGNbcu4C +10.65?îOòâhÈõ?«%=åßZ~?mÇ뚖?zàÓ§uçñ?©$`.)cE?©‡µxiÀ…?î\r¥A¡?±v±W
s?–¬ ¥?£.ëX†²j?£
µR  ?¤ó~ˆ\?ëL»F´ç ?©j(n²[?§‡C!Z>?™ø&¯Ñ›<?¹Ö"9=Áà?¤šê6öÿT?é¬a7R|¥?´CÍ Œq?'õ˗mBl?u»‹At7?ÈhËÆh?³îÐ;Ë?ìvDÙ•Z?´¤†é…î?™ÎÂÎ ?€Ã}Jz?ºU¿œ"ýÎ?´¥t<j?ê}žG9‹£?ÈY/*SÕY?°:ç+6©N?¾'À³—z?»Ø&"»?½Ÿ?~x´z?èïÇΜ?±š;ºà
?­Þu3ç@Ê? hçœq?ÄÌZԝ?®q/̕R?åWÇÓ¤éj?ÂüÀì€?|üö"kÌ?d!&1D?ÔÜ|€Œµä?…gN~úBAGN4FGL J2117.4+6159c?ïóWQºK°@!µo—g2À:²aç|À;ÔUÓq+¼@)Ñ,­Ýô@Ò¦-?Õɞoc?èÀ‰þ#r@
fr$àŠ@¼]Sm:k?ïþnÀ}>¿ÚkJw—¿ç<"Åý¦¿î-ë•å¯ó¿Ô}¢'¡Zƒ¿ï¡kTâ°dAGNbcuNVSS J211613+615920 ?âÐ3öó??Ì¡ÚèÅ?¤B¤òì…Ë?¢ÿ¾\^µ?××Cumé?ËþhÕpN6?âúcQÇV?ɟuEý:S?¶ÀH{ú	a?²¾â}U?Ô['>Är?Æ'ÖRæ?å/J?8-?°ÅÂÑõQ?¼™x<@'?¥{ÎP²)?ÌöNGØÿ?¬ùI½Å:5?äÕ²Ø¥?©
˜mL½?¼ÒpáЦ1?¤´…±š?п¸aÛ½+?£ó4T@U"?ލ¬ã«ê?ËvaˆR–È?°ÍfsÔ'?°(˜`W°J?Ý?'¶•Aµ?ÊéõÒ"5?Ók±0†|ÿ?ËT6©ñfÆ?Ímiñhì?ÇÞ°ÇU?ÝÝÁ€Î‹?ËI	"õ-û?ßü0':+ ?± £Rnщ?ƅ hjÍ~?­³'•Ó·?ÔÀÿ¤m¡?°­Ýq=b•?ÐÝÑ.'Òú?°ä¿2?Ì¥Ð>qT×?ºÐ¯ÁŠ_¦?àg£YOÁM?·'øÜz]ÍMIXED4FGL J2117.8-1521¿îE;¯"¾ÐÀCp'IüÀ;Çwù5áÀ<hP?³t6@ÌYjÕa@ÏãzŽ;˜?Ñøòû4¿$?¥OiÒ~?̧Àä6Jë?û`¤$âãe¿Öa·˜ˆ¿Ýþ‰Î´¿à¶+ —ºœ¿çRÜ{–yT¿ïüt$•
¿?ï¶ý!ÿ.IAGNbcuTXS 2115-155?ïuý­v?ŒÒ'DÌÉÙ?Ldb˜°A?DÓîQ¸?y6zV?Œ_Ë‹I¡?ïrñ~vÂ?‹?C'xÐ'?hiI'	ÐS?oR.(¬Ñ?a±6H…c?†3üÆ_b?îøÉüt?Pßpä%?GC™†q?~ë! ú?™ï‡T '?‡3Ácè%Ñ?î×~úål‰?t«±õµ?h1eÈò¥·?Sl÷©âŒ?¡ùöñŒ?€VÌVŽŽÅ?o«'?›È¼Q<y&?[÷mI®n™?SvtþfD?£þ{29î?›n½‰2?înX(Ç/»?¨AjYjH?{€"ý'n?‰³è|
$?¥ªy³?¥Yˆ€™LÖ?î(Á/¾<D?—ÝF3ïZf?†ÖfBmýx?ƒùûC®Ç?§¾Spíh?"
Ó4ô=$?ìgýUçÏC?ŸÑU!äd?yµ°XÔS¾?n¿Ù~öÒó?»$ºI'p0?Ÿ.«/¹AGN4FGL J2117.8-3243?ïÂHGu.ÀEïÚQÎÀ:z[ôœïÀ<M\ú¬Ùè@ ZÛ¯"«ï@eÏ?mÔ?½h"£¾5°¿šÀ>ÁS>c?ßX´Ae¥÷@ËÃw?ë€FvÜÖ/¿àÀÁü28¿äVóAUµ¿¿ät9Ûr­¿Íy¨7—¿ãý먰AGNbll3FGL J2118.0-3241NVSS J211754-324326?ï§b}=¶?xKRšù?Nú-DÆà*?=À0oŸCw?"7½ÎX›S?wnm£Ëçj?ï«í"'l?Cn¥1JÎ?UfT[kr?ZÞ=¨L"å?'WÔ\ID?zŒÒØÊÇè?ï>Š$ù?…€½lÁü
?e-o¡÷…?dX•e%øN?•‰
‡ß?""AÝ;Î?îý.W›?y蚾FÊ?bÑÐ-.«G?Leƒ@ª}·?õÕڒˆ-?y¥xxÎO.?ï%f*p/Ø?5$dj?fVhâ?ZEëiÁtà?˜ƒOöÐeå?ŽŸ*z6O?ï8Ù/±žs?'ÊB\Z™¶?^¶Ísq)ù?hLS¡äÛ?–ùm;Xñ?Wº]%ÎZ?îb]אd?"ÔƒÐû?rÑ
XýQå?që?i¥r¯?§€;@'J?"ÙÝ"2?ìåÙN:v?—Ñjùð‡Â?zô
Cå{þ?o5ßuDõX?·(¨b+»'?—ÿ˜^ؓÛAGN4FGL J2118.0+0019¿Ä\ñ— \[À?è">À:¥6nQsÀ<Wæ¯Ìâ@ø5˜hA2@ø'œ&;Ô?ÝíM
tÎ?ÚDôPÊ?ü@ÇÀôQv@SÐ|"`¿ßc[+J1¿ã­g¬·"¿æ*MçŸð¿ívjàžÏ¿è¦ÞHJG¿Àzz(ÓAGNfsrq3FGL J2118.4+0013PMN J2118+0013?ï¼›=™Ð?ª›D3sj?CcKÈO…Ú?Bòw×È?‡Hû›¾?ª›_D¸Ø?ï¨_Hÿ'?ƒb¤ê¢w?W8TiÀŒB?_KÜõ&n½?ƒ#-Î?îJì"?îô30â~˜?'·{7öêÂ?{œƒH^{?|ndŽ?š'yÀªX?ã®qµ'~?ï¹æ=·7?_v?]Ÿ(¶?AÆ
ˆM2G?*þË=\5?€j%¥Hª?^To Ñ63?V¾[N?‡ÅúÜ»¾n?Q +èۊ?Q­¾\³"?Ši$ï",?†'"²µR?îÎK*­†?¥ÿhÝ7sÍ?q'¾‰*?€(!S¯!
? öjâÄRL?¤%úœ†‡?î6½âÈu?›Ò¥¤ Ñ?'%»mUK=?"ZUnkø]?¨
²øš˜ä?™U©6è?ï?9%\þ*?~ÆÍ}Ð|?H¨ÝfµË?EH~é5þ?—S›DÏF?~q2»`3AGN4FGL J2118.2+5752¿ïŸNPts@¹p]`-gÀ9Á;ϹçÀ;™j×o@àçñìA@	'C‰ÂŒ?Â>ˆ;xQ ?Ä}þ&×Z@TŸCý…Ò@˜öChµv?ï"]9–û¿çÖ´âË;Ó¿çtŸºšñ¿ç8×L''¿è©ç$f疿ï¾àÅýüAGNbcu3FGL J2118.3+575187GB 2116+5739?ïNø&'?•©ç?cqY Ž?`ÏC?\ò?"²Ð6[â?";|q¯^—?ëؑù´ƒÍ?·–ãԊ¸)?|A£d!ÖR?ƒ'´?U2?¿wUü$Âò?¶>õèÞ?î#•'¢uû?˜$G2Ò?'5Dè×ã?€ýÎ'ºáí?©9VŸMÔ?•qy!Ñw?íétNƒ?…ÇAiú ?|Â;Éa·Æ?\ZÓL¤?­Ðv´ïØ?"úHúÓlå?(°<7?š=yc¼?s¿ŠF³3?pk‡š4y?¢nÌ4£*$?™<JoK"¤?ç*4]™}?Ɓ`ó_ލ?‹z¬"T'£?•|£–Qùb?ÐÏÁàEá?Åq%øô.L?ì^qêù[?¥¿"qiÜ?•§¨ÁxÝl?ã&kÔ®P?·¢†ÅäÏ?¡ÃÐùÒöO?éW‰×é?¤àÞÛû»c?˜ðRmH?§R¯BTç?Ç лY?¤C˜®}¥tAGN4FGL J2118.8-0723c?ï¾D¤سÀBhß½jYÀ:ª(҇ ñÀ<,=]…@öE(þüË@8\gßã?ÍuÙ`ƒùI?Áޅ†è!?택Âô@¢ašú—¶¿æpoiDg8¿ån8¿,Ñ¿èëõÈ|Ü¿í†Ëá•[Ç¿îèïwòå¿ïÿüoQÇsAGNnlsy1TXS 2116-077 ?ﶉ0œ?¢T8Äö?EŽ
ãiÂ.?@#*a[oQ?Ó*]Ag?¢c…ã?ï¬\kR<?€8xc?Y÷¸Ï?h	þXxx ?ªÒ9¤¹?z&¬Þa?ï	|äpò?Ž¹nP^Ÿð?n֔҂•?s<ߑmùŸ?›µŒ4p?ŒçðrLg?ï¥ÖB¹°]?dÅÖÕ4ˆ?Yàùn²5€?@[çüÌ?ƒNP$mŽ?be'jòÊà?ïÁ§Ô‰ži?",Þn?S8XoJk?Qû*\
Ê	?z^¹@?ƒ¥ŸjøŸ?îõ-›£N?›ÌÈvúÿ?nvá•>L?~R+àS?‹r$屃?˜ˆƒ©ƒ¢?î'Øô	?d؞q'•?xžØM^?xýëò眒?«êL½"Ž?œ‰Ì±™Ì?ï
ú6òå?ƒ6A8'£?m¶ìávDX?[d˂‡Ç?š‰Û¨¶+Æ?¹Û+%òÕAGN4FGL J2119.0-3317?äç SæÀFbMÒñªÀ;Ykã}é:À=!Iâ¢!@ÉH±Æj@ÃRë__?Õ.³R)˜?ïÔËi~K@ëÿÛk@ŸÖ
=UK¿î~ߧz®¿ØÌü½«FÀ?Û¤]Aúv¿æ¤Dî¿î1Ū™œ¿ïöF"¤ÐAGNbcu3FGL J2119.2-3313PMN J2118-3316?æ2Ϗ–`?Ä-9œâW?ÂÈ¡Þ¦X?ºõûëÚjU?Åû?ã&?¸Œ5hM¹u?å!å‰s ?Êá‡_ì_ö?Ì·ÜЦ?Æ)Ft?¾Ú¥×¯B½?´x:TËÅw?çZ…M\T?²Œe˜É?—´! †?¬µžçŸ'?¿ÿë™QÜR?§›"àɒ?隚"U•^?¬a=Ÿ­5×?ÂJÛ%U$?¨R]UQ³T?­*ñB¾d¬?™áäè˦Ÿ?áèô0¨Ð?Å}ñ{
•ä?Ê)ÿsÏ@×?ÁeÜ[hº?Î20nç?ÀL@­;¯P?Ý­üƒ"À?гsb«ÏZ?Ռ›ÕðE?Ο ö®?Ɋлõ?ÁA¸àˆ
?áÔÚUÔü?»¨PIL-?ÐS¥¶н?·æIHÒ?Èi)©
•?±# ›4?á"?[ÏMt?½ÌñÀÀ?Ó¬tQ$y¡?»)öž'aš?–îyÖí?²‰ý¬ÁÿAGN4FGL J2119.4+4652c¿Ò lȑdþ¿þ©Ü¨#$À;4ÒÆÒíÀ<¹?QN§@!~';ýP?ýBL
šµ?ÙzGĺ¯"?î£bۗjë@	÷ÿ=ba?óá–óÌëÖ¿ïøgàŽö}¿êæe$G?îÃ߈'3š?ÕW³%óà¿àb¥ç…µ·¿ïÿÿÊPËAGNbcuNVSS J211922+465026 ?èE%ª´t?ÀàÙÙ›Ø?š>¶Ê? Ã'¿ç?Ë£´€?ÀÚlr™û?È?uãÔG¸?ęäz	þ©?´Q¤	‡
?¶HØï—hl?çeîx€?Åo4¯J?ê·0û—Þ?©¶M›ž"q?¢Zå^]?"Fºµ¯5?ÃRiÜ_q?¨—û¨»7?ßpƒž@?µ8ø¹Í‡+?ÄlK´³Á?³J<'zÃ?ÖYW ð‡ß?¶=´fÅ?áô³·??NJ(¾Ì?D?šzP>‹õÐ?˜:LŸCfW?ÚpO•¶Øf?ÇÒ鉅5?·ŽQKëô'?¹`…V喨?ºf¦xTi?ÁWïÖD ?éÁa*;"?¨ü‡"MC?æÙí¾xºì?°âý¼ˆûÊ?¥Ýš\Y""?˜"²!'Ü?Ï âpë?¯ÔVÑ?o¤?Ì°3ˆM?¸³ND³B ?ÐÎÊ÷=A]?ǃ ý‡U?à"îwŸý??Åæ{	5³ÁMIXED4FGL J2119.6-1105¿ç¢·æ
áÀBñŒ~($À:oÍuhÀ<KÛ$~dŠ@9"v¢s³@þZäR%?»§!	K>?³Ó}kÃl?õN¨‰÷e'@édZ&?ïìpk¢æI¿çóZ4ÿ¼
¿á¶ôžM›¿ä~q f¿ç™ÌYàF&¿ïïÀý¶¤—AGNfsrqPKS 2116-11?ïñîLyUV?P?Xõ:û?"l¼>Ân?Eó?Š.Ì?YÕКô?N.¶Y`—.?ïëXÊá)?e¦7çiÝr?)æì3˃©?8¶Öîz?cÆOë‡Æ?c»"ôùѐ?ïªm/"~c?|¤3¢V?eYLȓ«¼?upÄ\g"L?€`äCþ\?psw§D"?ïðKÓ¤=ž?? Iž?&˜Jïú´?
þ1h"îÊ?\ŽåqÅ{[?=¶ÍŒ^9?ïãxM¢'æ?iv9]½Í
?4‰[·m®"?.œ'£éã?iö†¿UJŸ?iÝÇHaï?ï»eôÑx®?€þÛÐéA™?=nY¡ÿü?R#gÎo^
?€;	S	?ø[§3˵?ï_ˆóü^?ˆ€äF/?zo¹(µ8?"=™mɟ?Šåæn÷i
?zò|¸!?ïÔ7QrZÞ?^Éy.2Îú?@L¹à©7«?-¸ÅR]܆?sÚÀð]\?]@7ʑõAGN4FGL J2120.6-1254?í'*)Á'ÀCnş±áÀ:hß۝J(À<d×ؙŠ@ÁÊÍC?E@}!xö‹ã?ÀÍßÇPa?®Â_œ®Þ?ìܙÿ&ó@€×€ÚÜ¿åîO¾Úé¿ÑŽ)ùΎ¿çñÝþMx¿áõ!HÏþ¿êŸåãõ~¿ÓUžã/»AGNbcu3FGL J2120.4-1256NVSS J212035-125443?ïîu¾óñ)?R.-yá?4LHÊ>¶@?&-óU€‰?^og©ü?P|Õ˜öÎ?ïä›$€ŠK?j'ÍDecs?0WÅ/'ÉU?=Žaڕ?iY㾫2?hPG·
?ï·Ú›Ü-Ø?sG†ßŽ	?[háµÐþ~?b¥Z›±?}8yˆH»?phN‹dàÈ?ïá`ñÛ?I Î(µ?Atˆ®p?#^ڜD&Ò?jBĵ˜?Gˆ‰·&¨?ïÖ-"šV$?i)ª¤&?K'æÊs6Ñ?AhŒIÄ]ß?qwúìTX?f¹^¦Òu?㮝j{H÷?"е>ڔ?@É,uXî?O¨Æ8xÑ?"8ÃD}¨?"/á?ï‹
lŒè~?ÿ® å»?b£äùwÑL?f­Øy«øú?ˆ"kŒ‰ô]?|å"-1´?﫚'Õï¥?hß°/ÚL‹?WýR =H?D*Tž6ñê?'±8½ýÏ?füÒb[¿lAGN4FGL J2120.6-6114?ëÄ»m¡:šÀDžî|IýzÀ;!—rwíÀ<¸£ûó+@OYýÍK@/ªJè\?Ð/níôdÁ?ȑòƱ¿?ölaR*o@œ7^+œ?î]ÝÙ¥¿å‰ÚÔ¯¿ã¡Œý©äj¿äsƒðºèŸ¿ä¼27Š±¿ïþ N¿€´AGNfsrqPMN J2121-6111?ïè;Û£TX?T	Å67—ï?AÕÓü'î…?2˜ Àca?cN¯Ÿš+'?QŽoZCT?ïºJÅcª?v²ç$e/È?O`kävTû?U;ûBã?~îì¾£ùù?sz¸šöñ?¶š9?x
a¯ø̟?^×ø9¹{?XI5/oÜ?ˆSCU
?vCü«£§?ï´.œ—ó?\ÁÕùue?Tþd;jB?4cx‰³ìì?€wT™aÞ?[Ùý0«Û?ïʨ=Sü	?iÓ/@ûî?RðaB¸?BØéJÖ/>?v'! ö²?gF4ìíÔ?ï8žO8?"OUCLˆ?^Ž9<*^i?p¤ ŸŸz?—È¡à^&?'û°f
?ï5M["?‡56àÀ3\?k¬õ"€Õò?j4ÛÇÃûÑ?•àÀ£|W?"õ0íf?ï(­¨†?y¸YĈ­Ô?eñ'i¸?Ì?R'QP±r?˜?¥_à
M?yVA`(ÿAGN4FGL J2120.7+4428?î_ff€+xÀ<AÏ®)À:?±~'­À;¨iTWp)@æµ+E~@Q*Dw(V?ÇI/ôºQ ?¡M¾ú§%ž?ÚiœÁAS@d‰ÉAþ?ïþj~£ôç¿á+"}¨¢K¿ëáxU|¿á2Åð9¹_¿æyÂr«Ä¿ïÿîbHÊtAGNbcuB3 2118+443?é(c'ËÍ?¾m^蘰;?p¹ŒÚj?h³xÒtŽ?ÊØ¥pðáˆ?¾B'Ê?é5ö¯T?¹£	«‹šº?p€¥yå?rLXÂê˜á?ʤ%6£Þ ?¹CuݓÈ?è6ÜL¾ìÝ?¯°†£¦@z?¡ã'	},Q?"bÑÌßîÈ?Ê«ªŠ¥y?¬®	Bgç?íÑDÓfx?‹Â™¼*ó\?yôñ›Æ•?[T&‰ˆÕ©?¯­™Á¼á?ŠnœÕ?ä3¤éj"š?ÃðdÉ«?}&IwõZ?t™‡R՜ø?×$/ò'?ÃÍ3‹.-?áp)M¬0J?ÆÝ®WÓ?vRNì¡"?Xq²ÕÛ?ÜÇdøö?Æ°ˆÀзŠ?á&Y§LpØ?´ss·6¥?±#dýàµ?¢§Ù8Q;?Ùjh˜^Ÿâ?³"¦hô†?êPÌÏY¢'?£Kƒ×¨'r?'¹©?vÔ:E?ěë^ï_Û?¢àÌ(ÐAGN4FGL J2121.0+1901?ï´YIiÎÀ5>
 r~À8Šr©jÇõÀ;£ÊÖR‡Œ@¤Î(š@>Õ®Þ]?¢^/š;?­c|ö÷@ÞZ"Ê@
yñßÖ¿À?³mÖVοá÷u¢™r'¿ã‰-°ê¿á|¾ß¤@¿æóBýօ¿ëM³"íbAGNfsrq3FGL J2121.0+1901OX 131?ïð+³Pé–?Qcžos(·?(¨ÂÏØ|?ž×XÁô¦?\"y×¥J?Pa9¶£Ö?ï¯åªƒ®?…†qV?`å`³œ>­?jƒåµ¡l?šzwçÙs?hÚ0£æî?Îj9b?‡ÙUæT?eàÓ9*rŠ?u5ÝXrtG?…×׍ˆ"Ö?…',"³€Ë?îùt—pcY?w¦)y
ñz?˜±ëá—5?aìòYÎî?˜"27?t6\ñè!?ïÑw¬è^?mdlò·º?<•xÐ[ڕ?3Ÿp3öÒÝ?uzÒ2»¯?l.´0¼;?ïiÇÄÐ)?¡!*ªË§?}m€1û½?'z:Ò»"?–—fõ"¦¢?˜ãáeO?ïH#¼Œ|"?@õÚq8?qû¤×]p?|aÇÅÏÌ?'|Ÿ2Á»z?ŒŠÃfÄ?íãŽrª?÷ZKX÷?'ÀúòÕ%?zÊ~hŽ¨[?¨f¡½³?‹·‡IîˆAGN4FGL J2123.6+0535?¿7|Õ#ðÀ>µÜyÀ9é't1*DÀ<6¶NÜ&@½'ãɾz@
b*Vì?´+®À®l¡?"plN²À‡?àFǨ ž@
ònòÑï? œƒ¿â¨b8Yc¿èž»ýq°G¿â´ˆ"MÝ®¿áØ­«ŸU›¿ïÿânÁŒAGNfsrq3FGL J2123.6+0533OX 036?ïî²3T§]?Wðá,"Ù?.у%Ù±?Ô1¦ù¿?^Áuy~o?V"Bõg•?ïã€ÙëTˆ?ktT?3"ý"—4??X°vEF?j³ZÛü¿?iGtÀg«?ï¶[ªp×?pdßÃÁ€©?S÷7	B?@š;A?Ô¥©ˆR1?oUﵬã	?ïËÞû£yí?Q𐬁Ó?QyãYuÎù?3[Äðï?u²	EW±Å?Oˆ¿-³À?ïÕÞúk#?o™š¹ˆÜ
?B6¢¦]?5[íkêá5?rɱ™1u?möa üVØ?¡ëç^?ˆº¾œ!M?E Ä"èjÈ?V:šE"Ž?†G‹H·Ã•?‡–ʃݟÍ?ïtÚRFsØ?3žOý<ƒ?bN"3ÆÕâ?bªNŸ??Ž5âéXn?€Gž; -?ïtùôùÎ?p¼@ý'Á?iX'Üi|?Rö¥m 2?Œkbø#Ž?mFµ'>šAGN4FGL J2123.8-3148?Æ»ú.QCŒÀFæÄŗNÀ:µkÞuk½À<KŠ·~‡@Ï¡ê ó*@™cˆÕý?Ô]•\s"?à¿-§Ø÷}@0[b&eÅ@^lg1g¿æ"íٌÏ?ïçô÷í¿ë/•XÆ¿ç2UB&Á
¿ïîû.	(¿ìZVÆy÷AGNbcuPMN J2123-3155?î0úÑ9et?©ácÞ{êÀ?x*w>z5
?x	Ìjj?©ëª&?¨}֔}¤;?î£ë-FEp?¡¡Â‡-ï?‹ø+d «?Žºfxv?ÿž>¥´?™æVl7ÿ?í3ǍrÄÄ?Ÿ¨Ç-'_Ó?˜f¾XžZQ?Œº.ÿ5Äw?°Hþ°6Î?š¤€ÀiC?îJé)Ç?†¾¯"£á?"ö›nч?x¤"ãã?¤?ð ˆ‰?'Uþ-†?ìù®Br?®'†¦ˆüz?—Y÷Â?†Ð²Þ¯»T?´¬º[ü˜?¬)µ°üa»?ìéqØ#[é?±0ª,¥?š/y8|Óx?¢CmÙ?²('ïÙ?¨Ð+或¯?êЯ€
ÒA?¬ài[À?¥'âÓÊ?–'gÐ?¾æ'ñ‰Å'?¨s±Ã¥ê?ì>"fµÓ?Þe¸Æ? BÏì
›?·ìË,Õ?µÀÉûøc?—Çt
x[AGN4FGL J2126.1-3922¿ïç†p‹ÈÀFþ"ž­Õ'À:µ~Ư|ZÀ<"ú~Ù@ÕôÜ5uƒ@™ñ®-¥?¼A<á1ޟ¿£²€f­?çÀŒ¢8G@!ýŽ?ïý¸ýâïN¿ØL9)y¿¿çê¹aµý}¿áY3BL«ª¿ãùïzv¾£¿Ò<ªÏ'AGNbll3FGL J2126.5-3926PMN J2126-3921?ïÏïœZ" ?ljˆc)-À?BUÏ,Ÿö?6µQ.á­?u½®^XÃ?j~;tiA4?ïÀ ûçÜ7?véÐa)'/?Pv©'?T¾k˜!òá?{í¤iq¿?s¹Îù8ïÂ?ïSiQ¾A?‡‹¹¼©	?aÊ}­Kó_?b9"'GŒ?"Yk|t?†Ô¬Xý¶é?寧'ä»?`]£"Ê$e?ST¸ƒ/›?5ßl#e‹h?ƒêÈ*®8?_–EùŸÃÉ?煮xò??wfP]çÅ?Q›(,GpR?D»É£"Jn?ƒ%|Ï$)?v¼Þ¼•?ïa6~Iæ?
=˱|Œ?R"<­µ?ZF-oÿ‰9?'¶%p›×3?ŽnˆÉ½£º?îÙÝ`1²Ä?'aÕÄ(u?mêûŶh"?hz1ü|¿Ñ? ƒz<iå7?Ž´<O's?îß÷džˆ?ÜPè?nãÅ
›?Y]g'¹À? R¨ns¦?~<Æî³ÒAGN4FGL J2126.3-4605¿ÄSš7_xóÀFÏG0@9¬À9kæ'øÀ<5/Ùâ_@\XúÂÿD@Aà?pXX?¦ó5—;›b?¥P(as'?õõ+á/Za@Àw¥("¿ÍßÈýà@¿ä/D%ɾ%¿èèSpÀ\|¿ãOCÕAæT¿ë`›KJ.¿ïúÕô"»3AGNFSRQ3FGL J2126.5-4605PKS 2123-463?ïöl¹šHŸ?G9?$?,ÇuJ³?!úòÌ5ÀÃ?O<^çH?DE—¾@9?ïë˜2
q?fØåß]—?0ˆ7®¶s?>´Û·ÉÌç?bVÇ!f&?d®|­Àì?ï¥øƒùŽ?ÝŸ'ç¦m?_ßTSZ?lƒò¡V?'…ôi}€â?¡B2:þ?ïþÅÕ"Ý?
S[ú>ù{+ig{>é…³w^? ~˟"?
/Xϼß?ïñ^=3Mq?Q¦†úÌ­?5·ëÛXf?(†Ÿ¿Xuq?WՊ¹ìp7?Oª‹×G·?ïÃÑÉ`܏?…7مùÆÙ?C$cw6'?`†q¡gÞ?{²™ãF?"eú]ç*^?ïtV×'C¼?‡ÚÙ/$¾x?`¦sf½ðÚ?g‹Îÿþº?ŽÀ­Y¿äÝ?‡ǬXa?ïüþʺ'§?+ôºÄ*'?Òìä…Õ}?
é¼·dIá?3TîΩ†?'6ŒL#¶AGN4FGL J2126.5+1842?摩ڞ5yÀ6m»{k±)À:ÏáÕr¼À<wª¥æ¯@ 4‡†Êµ@ÛÄÒ,ˆ?Á"AÞÇ¡¿¢|ÉCI?äMÝ|è‰@aŠžÿßõ¿ëä¡Ý4ú?ïÿÁeÖt¿êÁj=¶nç¿ÉŁÿÉú5¿á*«ýI¿àaO`eprAGNbcu87GB 212407.5+182753?ïÖ¶Hã?fôE/‰®^?ALøû*¸x?5a/·»š¾?r{<‰¥Í?eøkÄJ^?ïæõUé&Ü?iDä7k?1
]ñÖ?=¡mYÆ·?fç¨ilàf?fíÝ,…2ô?ïYFŽ•ë ?"(œ¸O?Ã?c[(/uÍ?gí«GùŠ6?'kÉ*?"w?ƒrÞ*(ƒ¾?ï°öf'|?aÅgñ0z`?Xb·þßš?@þ¥Ô'?€¶'›,È1?`ËPã¼-?ﺠ"'Â?sç‹ yW
?X2¬$¶˜®?Rl®t]"?|£?qÕuêÊ-?ï¬À©d#&?"þ½,=B"?FÀ;oóÒþ?ZÖÜìÀ¿?ƒcÑï :?ƒ²ò‰‰{ö?îü)>ÆA÷?ŒÉ(´qe?iÉ,1ËÏÙ?md"¿bñ?A²Ž«0?Š¤ O8žî?ï*pÁß?~Ž°Øņ?rnú¹¹?b"1L(è?–)ç?{ õ€b¢uAGN4FGL J2127.6-5959¿À¡ÚSŒßÀE=¿H˒À;X?½…1-À<Üdçá%I@ š-hC
l?üuãTΎ?Ë:'C:è?ÃÃú€º$ª?÷ځNš@""¯ ê?ïîy$¯ò¿í:䜸2?ސ'¡»ý¿àʐ¢Oοåñ6;%¿Ñ²'¤\ìAGNbcu3FGL J2127.5-6001NGC 7059?ï¾ì]@?zšë†$â'?>-'Û¸ß?10Øšç?0à)ÄG?zª²tª?ï–à÷Ò	"?¾8NuŽ?]J£ûdë?]ÄcÇ¥›†?†§8ÈÜBÛ?~åÅí¹š)?ïM_é8'?'qíDôÌ$?\Ѭú	j?R€‡Ë£?"†è'†–?'%T²c±Ø?ïó
N?vq:U•vˆ?a¡\?N(«Gs?šX$Öºg?u–Ó}(gX?ïu:x2'?‰˜¦!ۓ?Põ"¶ț?MEiÖ'?IW¦žÔ†?‰;5óóPq?ïð¿,?"‰íÛäbƒ?f͘³meÁ?pøl Ü7?›HL+Ô?'˜¸"Qš
?î±×Ýh»?'ßF?dPÊÀԁ,?gQþ'­ëõ?£u€¼|=?'eÛ[mÕj?í}ÚÊã?"ÕÚ$"­ù?p[Åú{ÖÃ?d£c¥€Ó?³mN:Š:?"‹`tH¢AGN4FGL J2127.7+3612¿¹AlÀ%ùÁø]tÀ9Mo«‰†&À;ËüÞ1@Ês×K?üþ_·¼^?²a>‰R¥?ÀN®ä¯l•@¨!ò™0@1<ëج¿ÎÍÅÆ[¿Ùú$‰LD|¿Ø~¤`GŽ¿ßŽ?ÒþÀ¿Þ4"ý#Ö¿ëá& þ'ÃAGNbll3FGL J2127.7+3612B2 2125+35?ïã¦]d?\¼YûZ'?B?–†PNê?:ˆ¨0‡"Ê?gÊFÀôÉ?Y®CMžJ¯?︳4l»Œ?ˆJ"usz?@}kÝy¡?MŠÔ·"ò?€Ë\<fl?‡%ݝ%È?ï•àeõ—
?yL÷´¿Ö=?eiTê'z'?j£í#êö?…-'E¨¤Ñ?t´ûC•?ïY0'»?sjÛh`"'?_}"{d)<?>
ë¢9I"?š]ú?ryÛd‹?ï¿á¢¥d‡?t'¦™{¡j?SåjgyÏ5?L›í{Ø?{Ô'Pþ?rÃó¯l™ ?ïO¥½‰Û?žŒçF½Ý?Sòq%Iú?eæé'X?"Ì6Ó:tý?…Êns‡)?ïZXºg€©?ˆ)¨3Õt?mš{-S8w?v/[ûçâ?'™Tœ±É?ƒ‡.æ#T?í÷-}*'é?ŒB¤Ç?piï\?®-?W0Ø
¨°?®ê@Ý0?‹}´JoÆÕAGN4FGL J2130.2-7320?±ÕÖ՜ü'ÀBmß 'áÀ;JòÌ:֖À<Äô,'@É{ôíþ ?ý=¨!ò™?ÒáÍdø'D?Ԋ\¥Gw¹?ø*²ái<@8ô‹(?î˜32\sž¿íè†1		?²|Ç£m-¿ækµÆ 
b¿é/ôq¬¿¼%p§ÝÕAGNbllPMN J2130-7325?ƒ†‡Ä?yÇë†)?_°²/ł?T	ñƒ­úp?‰¦ÈÓ¯DE?Äú©}Š?ï~"d²ma?†‡Ð†z3÷?fۊI)r ?kòc"!݇?Š¤D9ã?'\§£Û?î\tŸub?—!hËê{i?|~Be/'?{z	¬Š5Æ?¦¯ÐlÞ]j?•Ä89ékû?ï&>`7ù?rxé«ÁÑ?b¥è5¡¶?G¼þ¼ö£Z?˜ãvñô°‰?qu—õ'?îï<Ñá#?"úF2¥?s­'Æ D?f묋ä¥1?-&
a»§?"l΀M±?î®ÿÜ2Š0?ž.®Ç±¸}?u°×ÇÔI×?ƒ!™T½®	?¢YçH–JC?™9 –«+?í5@¶ÿ[?¤Ér?ܐ™?ƒ7D\÷·è?'qÃÍ+æ?³ï½ž?¤Uâ-Þ¿Ñ?í¦¼ÿŸˆ?»¹Ý\?n¸ì路‰?^üe
*¯6?±ÔW¡û³'?UJèºÎAGN4FGL J2130.4-4241?ï(·ëPÀGUž™ À:•êњ'çÀ<t&"»@G6¢0—@Ð#éê?Æ?a>ß8à?›ÕW	ý?ø§°³'@Ù{´Qy¿éæÍÿÒ³—¿Ö"š.¿çå¢'<¿ã8?ân¿ïû›÷Ì«¿ï=I6ª·AGNbcu3FGL J2130.4-4237SUMSS J213017-424319?ïNÛì`¢?¶1]
S2[?Uæ`>Ö?ñu曆Ø?†	ÕN£˜?³Ì+«9z?ïì`£®ÆR?p2fOWež?-wƒEús?F¡¶sŽ?aÇäZ²þð?k¨3Jè)?¢KÍg?'µ#zåJ?`Áúš;.?bA"ªdñ?…ËfêF™?€YIüÝ?ïû›VT—Ô?%"`†¶Ý?zL½ïÌ>ôazÖBŠ?@1ÿ´?$¬K—<ûê?ïÕ­d¸Íx?®'±r_?7Ü[ÃÙCo?F™Ò{˗?s«‡ÿҁl?®
É2"š	?ïÈüXßä?!Ú¾M"<?<50
k¯£?KìÞÍàu?y¾€v
‡é?}øÙt•É?ïcŒ'ô3Ä?‰ÿñ[Z@T?_«Ì§"?_?$æc×?'"°ù\?‰¾…öÊXF?ïô¨´û°÷?EèœVáíd?y¹å.?µ]Çô(?TÆú£¾A_?DÓîí/uAGN4FGL J2130.8-6623?ïü‰•ŒæûÀD È`VíÀ:@.A[êâÀ<Äa¢—o@1O¥"´Z?üØ´|sîå?À'ý]¹C®?ähY …F%@ }(®tòñ@ÿ9Cm"¿é Û!¤??êìȀ6ò¿Ò//bÄw¿é.äïÙA¿ín—ø¯©¦¿ïýÑò¦{)AGNbcu3FGL J2131.1-6625SUMSS J213038-662356?š¢uÏÿ ù?¨ÛJíMÇ?îÛ¥²E|?¬%i™g=Ó?ƒôªõ#?•­¡R9wŠ?¾D¿jÂQ?¾Ku°l€?è·êöê"Ã?Á¬"­Ï0ª?»ûèÝéC•?±²¬;z?Æo<ßës½?±Ëbʬ_?æº/¸n4Ö?´.h¯ÀJ?½PôÒ?¨Ps<=?ÛÆh8V;?²qÌp­?ßgNÁü\?³8¢ˆhŠQ?³K…!ƒ¨?•úfÿa¡?œ5>Ý'¼F?¢ø:ËÄ>R?îºËºAô†?¦éÚÇÕÀ?ˆâ"ÂñÕæ?ŒÄ¹†]¢?°a¨ÖªD'?³+Ÿ= ª?êM	œr"C?À‡×9ã%ª?½6
F2œé?¸w$nõ+;?¸åÁH1?¦‰'=eç?é0Q?°›Ó|d6?¾}¸ZÊ?¨y
—t#´?ÏÓX	ßÛP?±9›šÊ?ä@B…‹š¨?µº;…Õ&?¾W;¿ãt?£4boLCDPSR4FGL J2131.0-2746?ÚlEØD$ÀFì×à&EåÀ9‹‡T¸À;ìh?"zN@3úÑíÈñ?ùóúˆÇº>?²¼;7ó?¿	Hþ÷l^@+ý´Ì%@
§&5ô®"?ï'v Ùó?ÁDµüü•g¿ÉΆö©À¿ÜZŽâ™¿ØÇÓ~AÏX¿ãcs¢¡AGNbll3FGL J2130.8-2745RBS 1751?ïíéêŒGÄ?RO-¯üŠ'?A!±9í?7À¨É"?[£9M¼¿?MÁk'%W²?ïÏ_ê~ìù?w´W`2ž?Eb8'ò/?OdzÅoœÈ?u£Ã³Xe|?uaŠuÊ?ï˜öõŸ?~ŠzƒÝýB?ce;f.u?lˆe®ta?"èóã«ÐB?z³žlV?î©îw"]?€"/¿Û?hqŒÁæ0?N–"R	÷?£ÚLC|6?~ð	êÆÒ?ïÑÕÏøÔ?n°qî¡8?[G7&PÚ`?[ôÿ°½y?pCJ%Ëy?e ;gë¼É?ïc3ʘü!?"@*´ÖÙ8?]nŒk+ô°?rüªÆÆi?'êy?Ž?'_r§'ö?ïW†ÈNÁ?Š½è+ÕP?mtØù¦6?tó7èea?'`¤	Ó÷
?ˆÙSò/-?í;PȑÌ?˜#èˆ,C\?u½D‹¨?b•¡ä€?´ÔMé¶?—µ‰Â¿‹NAGN4FGL J2131.5-0916?ïэ¾fyÿÀCÖ@|ÇÑ»À9¥
œ;5À<%Åo@	_	ç?ÿÃnÙј?°gÆä*Œ?fœÏŸ‰'?¹ìÒў˜²@
-:×ÂI;?ïsÿi­¿ßD¦âÔ¿ãÿ•g0¿ÚE¿'Q¦¼¿á•Ÿ¤u•®¿ÇôwáùþAGNbll3FGL J2131.5-0915RBS 1752?ïõ©€Ó‹>?L	0‹,?"5­ðË,â?/úÉFV?RfHÕ£q?IWÌ¶k?ïèIdåo?k¾×cx#>?.+F—ñž?=ë[Ҏy?eÍ©lþŒŠ?hûEž)R2?ï³ê¨¿|?v
F"δø?OÂVVçü?7kͧqµ?	Vµ(IU?uÚ#(4?ïËÀ×1eå?Uûq0\ÿ¶?G5:†_£æ?*9«2fm?w8í o?Tmrs3Ú?ïî¨@ó²Œ?Rìê/¦dB?2§ùHø·¢?$›&³b?^¨ )õ?QŒ‡ÄLN!?ﲊ뚲?ƒà@oûFM?Aþ£Ÿê?Sü0ƒ#¸?'Ku<ù ·?'¬¼íIږ?ï{Ǔà¬?€À"AÚW²?Y'ƒÌ,?PUçO'úK?ì»4z?€vÍ´Ï»?
ðZ,?pês˜ªc?[®½eLE3?F7H•"Ž?‹%e¢î˜T?o$¡$öUAGN4FGL J2131.7-2515¿€ÏQ-çfÀF»F^‰"SÀ:YìÝ
Œ°À<ZSÆP±É@ nYÎÓb=?ûÈF¥Ö¾¾?À¸ô'ڏƒ?¿×´ÝAäý@ÅzxQJ@iÂß84O¿ïŽI9.õ·?ê)¯[¢¾¿ÙÁa3Ϳע."'AÜ¿àÿŸY¿ÕŸç't1AGNbll3FGL J2131.8-2516RBS 1755?ïáÀ|‡e?Wèú¶Ý%?CaÝÅ{ˆ?8ÅÖv8l?ig5cÖ;?T±м?ïÁðžÊA=?y×ýÒ.-¶?NxþÛ¥Òõ?U4Ùí™æ?{8Â"ä}?v0q'Œ¹?ïŠÖ¡Èù?nÙHŒZô?]A&;Úb?Eâµ!³?‰Ñ¥•Œg?lMþÿ7¢À?îé6BÕ?r"˜œ=.?q.=Ú<?P0'ÇôRi?ž"
NèY?q³(7Ž?ﺻ¤þžù?kOæwaÄ?aSOÇVT?Xc&#ØÝ´?yø£9à\[?d‰à¾š"·?ïFñwbH[?"m"ÂÆ¿?`Nł¥/?gð
dY«I?•øa~‰Ä?'®ÿ†)ó?ï'«ò{vÞ?€f)9")R?hmGa¦F?X|kÅéÈ?—üØÎЂ?}«!'¹ß±?턠ŒŽ)Š?‹"˜¢ðý¦?o€®u¦?i&oað?±º
ªf<?Š%8[¬.AGN4FGL J2132.0-5418¿ëp´7¡úÀFliƒQX¸À:	²Œ¯¦KÀ<jńÙîô@Mä@Ü¿@G?Y²#?¸y€Ÿwª?³ƒS‡ªó?ø9ߊ>²Ã@ó–ßU§?î+|…Œœ[¿áEäEVJ¿ä^_[Û¿æIøÜö¼¿èñÒÀ¬­ó¿á_L@ËLDAGNbcu3FGL J2132.4-5420PMN J2132-5420?ïê†p6'?XŠ˜å‰›?8¸Šš/ðÖ?DAá½i?bbÐ-Ï!?TÌ5¹z~"?ïÞLK³Ó?o&k'µÐ¸?8ìäÜñW¦?BÎ& Ä?n–Õñ×?kök!f?ï¸MpÃð?rã[ÐÒh2?V*ßÜ-?H¶NQ5îu?~UEìó,¹?qŽ5]"È?ïà"ÛTØ}?I†'n¨X?HQæƒÜÏ?*ª±ÐžÚX?iÈàÔQŒ?G`2U'?ïÀÀ=áü¤?qȑ'Š'?QMÆ+Ì?EghVB?{Lo­'?oqšØ¤?ï¢~1ß 7?…¨bE€£æ?I'ÙQL?Wڄ,_Xz?…Íõé<]?""ßw÷—?ï~ì5²i?{l§G&
#?gŠRÑùz\?fÄÔ´6xÄ?Šbfýe
?w‰ö®žD?ï¡Ûqw³ã?n'w'¶ZÈ?bxHü—ñ?N3`X'¤!?'ëG<ÛK?jtt®?#pAGN4FGL J2133.0+2610?ÁA¹DõÀ2q»à~íÀ:×Üßi‡ƒÀ<?‰›ár@ù¨çj\ë@¯ŠÄê€<?˯æ8óg?Ör$u*Nˆ@ýæJLT@´²@¦(?Ñ
8þyB6¿â¨˜é_¿çMFkE¿äã¼gú»¿ïþ€¢§µ¿±Y¯ô¤ØAGNbcu3FGL J2131.5+2605NVSS J213252+261143?îè¶ø¥Ò?–^ð"_õ‡?‰Ù3þÙ;%?ƒjjò²"ž?•ü†ñÒ&?'÷¨‰ÆZ?î3|`Æ
Þ?®Gÿ0ä±?—Mtçƒhr?›Æ˜;†Ïú?¡!|nê?¦'ióeP?ìƒX'«Ÿ?¤P­éóÿ5?¡šÝd?"Ež‡Ïs™?³ÍaHõ?Ÿj®…ËÐ?éëWÛøӀ?™ºÉÆvá?°
þ½6?ˆP/·åD?ÀM!0|I¨?—,ÉÈǕ¼?íÉ ?{?¤öøáJ?›Ê°ŠC\Ã?˜F1/€?¥€£ÂQ­?›8øú:4?éÐsÃÏ«­?Áô¨ë#Ø?¸áøýq??¹Ë…¤ðñ?¸šhâÇ©Û?´È3يñ?꿈‡‰²Ø?¨'Òv½ž?©ƒWÿ>¿?™ÂcØö?½BÄïà?¤‡óàÕä?ß\çÄlM~?¨¹éz•b÷?ŀMøÜJC?¥KÆï;'O?Õâñ>¬¢?«þ¶ÙåGAGN4FGL J2133.1+2529c?⸷äÞ;ŠÀ2óNe¾ ºÀ:«ï}Ѽ÷À<j"l
ë@ ¬³Ho-?þȼg#ûˆ?Å'Pǘ°?¤Pl ‡‡?ã>Ÿ&Kn@û©Ã2o>?ïúޝڛí¿×Ô¿?E-¿à£^Caÿ¿ÎR$zˆ²A¿æ»Ê`áÂ'¿ÒƒSœŠ9ÕAGNbll3FGL J2133.3+253387GB 213100.1+251534 ?ïв±(è"?fm"‹ x)?75ù3?)ôEG>ü=?v3Gº… ´?e·'sÿ¯å?ïÔK¬PÖ\?rëÙk÷4?A[6YôN?GòK|æÝ?s®ÉÃ4H?qe'Õ|î?ïz;$G?yNÊ·uõ?Z™gª0ë?FW @Cê?Ž	"/œr3?xä÷1½L?ï[—--µ›?lö×,™0?c€ŠUa6ù?C¤eT'Ò?'	"?»?l»MÓ°\?ï±RŠˆÑî?wÇìðY?D(Ò2?6Úä‹Hw?'hۅ}%?vcµÕb<?ï'ç2ÿ†³?‡} ì÷Ÿ?SØnù5Ó?[¤i±h{?ŒË%"~<a?†¼Að§?îÓ Y¸iO?'d¦.
À™?f®õ±}}
?dõQF]Î8?¡[¥4??'ËQÄæô?î/Yæô?†™ ¶¦¯?xnr¬Ú?b‰nŽ:?©ú.@€?†ÒM{oUAGN4FGL J2133.6+1439?Ïë$¾GÆ5À:d6†¤ÊOÀ:½|·¸À<" ()ö@@Ã]NÞ@ךCÅ
?Æü7ž}¿®$=®X»?äµÎMÖL¨@c']çç°¿âøâÕLοë]
Œ°}¿å'z¡0ç©¿æ9Mß0ýy¿ïæ¸f
{¿ïÿò> wAGNbcuMG1 J213339+1443?ïïîTùW?Z9B"˜h?GBƒë?Eæ˜Ôæ_e?T¡VŸo£?S8ä(K?ïÍtmmÊ<?xeÆ3M°È?GY#*rT´?V]¬–
?vZ¤ñyoý?u-1¢t?ïdøó¦?ˆyrü"œô?^ED?a™b—šÕö?'œìÆøY?‡ûµmŠœü?ïºJ(-W?axÝÇý?Kô=DaÉ?5Ú½+x?húð£y?`iÂ7±À×?ïmâ¡Lý?µù'±X?~IV¹‰ÉÏ?§÷èNExÔ?…bÎ<Ÿ©º?ª'6¤Íli?ï`jÚ¥Ž¬?'ì³®)ì?\g-ˆt?o•ÙgX2€?',2øu©?'ƒõÑ~?î¹@T:†?•uµ¡³?hÛWãº?p@Æ澙?¢ÞI/ ‹ä?"q'ÍàX?ï.—2>Ê?—P5èg?f­ÝR¾Ú??\!-[\¹ì?—j1wjj?€b dÜAGN4FGL J2133.9+6646¿¯ïg_g¿@%ù
{é…jÀ9Wòw@ÝÀ;òd\ êÇ@åÄ[º@èà(Ê$?´"54Y©?µ@b›«—ž@
Ú\ˆ–@½"NXӁ¿â<kU¹où¿Ñ´ådô y¿ån oQ¿Ö'°œ?':¿äé2(q8R¿åFÆÞvB|AGNbll3FGL J2133.8+6648NVSS J213349+664706?ïî}å;·?P|ý"§‹?0&Ód>#? w¯µQÈ2?^ãëoÈÔ?NÝÙñµP?ïË27#œ?€¶Ú¼Ö?IMY¦ù?S®ÏÒ3ëŸ?w=9057?}NÜý?ïšrü£–?uU#c+?`
¶à·?]Éj'ÔA?…_ÓToPÂ?só` -r?ï}WD=$V?hÓÀHJî?f³kV­E?G
z{ròN?ŠýT*ÙÛD?gd|Z‡H©?ïÞ[aikB?b6VÌQ?>¦2#iH?0d(¼iU?mÏÎw°Zb?a9!&ÈÄ
?ïlmõY't?"£Þ.-–º?b¾K°Ò£*?t­y×N´X?wÜw¾?''ƒ… ?ïW½¸v˜R?"´vhÞ?h,sDÕûÕ?fjO>؉?'º‰B"S?'Õ[!äI?î'ö
nÿù?‡``Õè0T?€žVn€ú?gŒWìlü‹?¢©	ÁMQg?…À¹+âuAGN4FGL J2134.2-0154¿àÛy"À†ÀBDzd×ñÀ9àR»Ž·À<I—"Ç@Ò¤e¥vG@DfBT?ªýd©g?«èž ¥¸@=ÙÂ~•1@‹–'(6*¿ÖóünñO¿ãaþ»Ý;¿äîvjÀh:¿â#•›Þx¿è • ãû=¿âᙹzAGNbll3FGL J2134.1-0152PKS 2131-021?ïõµ`
u£?L	[¢´Þ?$œK0¼? ᯻‰0
?R½¬â¹V?H~¨‡x"1?ïáÍ#x™Þ?ptj2Yþ?9ÿ·'?‹¾?I—ZÊMí?jòåÑÝ®?lnFcN?ïÂWS|?fú˜…Çþz?Rm…4¡ä?>¬w[¾$?zs8æQÊ?euيC:?ïê$ùS?ELÌBÆäó?? •kåÚ;?$t"å?aççv™~à?BÇ![mž?ïꬣ%xN?W²ÿ"w£ñ?5S‰}4d?+a~`à?ó?b¯²£ÁfÃ?U«FÓk§å?ï§%»š?…NL	?Fì^cOW?UÓ[;úÔà?"Çò¼X\ú?ƒõAT~Ê?²šF"?{o~îh˜?_þÂåéL?bVÒp"Æ?‡"{%ð?x<aÛ(?ïǔæE]œ?céN't8a?UV*z®
?B¶‡V0‰´?vàDäòš?a‡£g°šAGN4FGL J2134.3-6511?ؤƒ6D¤dÀDc¡À:Ç+×_gÀ<aýõ}Æ@Zt¥™W@Cá8j«?Ðe¦Ñ?•ÿ¥DÑó?·™¿¯,þ¼@ª7îý`¿ìÒÿõ5¿åk›#ÝTÚ¿àm>K?D¿åNìóà¿å°¨t'ð	¿ïîW–¿Ê†AGNbcu2FGL J2134.5-6513PKS 2130-654?ïÇÃQè™Ì?nȇÙç
?;RÌ"|[?.‰§fU̸?zmü}–8?m—õ:æA#?ïÐi^VÜ?r!9Ìé¡?=žAŸN?F¹c"y=?uñov¶çÇ?p'D',­É?ïj´o;»?€÷"ðr©Î?]ì'%?`K?.—*?Ø³N»=È?€F¦Ñ:B»?輦ošd?cgrÇÊÙ?DžÜ1Ì(?(׫mĎ?…öJÓš?c9RÉ$)?6°…?'åÇñ›?IîVاh?@㤤z?Œyí_z ?'[ÈeMyh?ïqRèÜ?Žp/µFÀ¦?QÏ)=oé?`ÏNn7j?¸Ë͙1‡?)èÎähÆ?îÌØË*-?ÎŸéGŠa?iFë4ãË?f"<8‹#ï?¡©ÃÚ¼2?èkòhþ÷?ïÂU"Jê?ƒóóó¦W"?U%çß?FïSae L?µcñäUÍ?ƒüçvÈAGN4FGL J2134.5-2130¿ét}JÀF‰Mçê_…À9xˆ3?ÈÀ<¸_W~l@†Cmqs?þÙ²"ý[
?°Ï¹Wf?²Gšs^F‡@¨Ÿr÷@)0Ôßù¿ïëC_Ñ ï?ïÂîþGn¿Þ¨èèŒF¿àcª2n¿á½?[_¢'¿à*MTAGNbll3FGL J2134.5-2131NVSS J213430-213032?ïù%+™Çù?7ÀaÒ8O?¤Ý\7äæ?¥+"
'?G¶µÚ¨»?5ã«æÔ?ïà¼ãm«?pËÒKÝ?8è[×ñ$?EhÖ`žm?l&4¤X*?l|c0Tö?ïµhŠ¶…k?ukQÓIx ?XÛÏTžÈ?e¬`CÅþ?ÆÊÍî´?qÑ)sÛà·?ï¸ÑŽŽ´Ê?_€hÀ'½–?TB'mt·?9MÎѦÜn?~†˜
"m¾?\}Þr¡?ïòÄ­é¿?MåÑ8-ò?0:JÊu¯?!Pò±eî?Vh²%@?KD
ºô`?ï«_À7›«?"µX¾'_Y?D'4<‹*r?S.g
ٜ?ƒÞü¥Ü‹Å?ƒ•­ž*ÅH?ï"avg]?ç«ýÁ?b"¡'Dç??h¤ú¦|®?ŠFyùûŠú?~-÷ý'˜:?ïiÜ×JÃâ?wŽW¯?d°¥…ÓA›?QÊ֙Oï?.P`űˆ?u³»ózz^AGN4FGL J2135.3-5006¿ØcF'FÐ/ÀG3)¡¹ù‹À9-w9ó@ÕÀ<AÞÌ©'^@])DÇÛ @'bå¨eå?¨µ#§"Ç?²Ë›^ëÈ@"˹§V@_kó™d¿Ðð÷¹à`þ¿áîÅæ(¾e¿æÔ²¡¨\¿å§­ÞÊü¿çȈd½ïº¿íÃz=³¿¶AGNfsrq3FGL J2135.3-5008PMN J2135-5006?ïìÚyãØ?`¦éJö53?(%6Ьº†?!1[V—‹?a£«E°?_é,€óÏ«?ï×"š#?v;gåŽB?Aö>˜£(a?QôlÐ@%[?r4¯åh¼?sQ¨Ç½v÷?ï¼ñ
sÜ?p…a |ÝV?RÂ[?:æ
w˜ž?}P–ÂåóX?p6‹9"?ïãsú·?Ln›È1Š)?Qãëïd?7<I¦«J?cÿÍ)çΒ?F/€¹D§?ïÂ
^Ûû?|ã*z.œ¯?=¾ÜÙ¢ÁC?8{›y?}°8?|-¯ð?ïÁ8™úh?É_§Qàj?R£¹81~	?e¹Õ&Í?‰{:©Œ:g?)V`jì?[sÝâ?{šÜ÷$¬¸?^ëYÿG—È?Y^é·ï'?Š}ÔYB˜?z;«(¢3?ïµÉÆCW?n.æo—?hèWhVáz?XTWjŒ7?xýïRµcâ?fiKì'+AGN4FGL J2136.2+0032?ÑV°Z7^ÀAÊdÂø7µÀ:÷Q۔çÀ<DFŸ@2΋hÔU@dZ˜Ó?ÀüÈŠrà?̙}jº@ FÇd®@ج8'¨f?æø¾&@Ü¿éòÚ/­m¿ç» !³ƒû¿ïÿùµc#¼¿î¬¢ŠÙã?ïù!bü$AGNfsrqOX 057?ïø‹â6k?NÇÑX½äí?4£Ö5Âf˜?6s*ãç?CäŸ´)x?F®Óåû¢]?ïÖ8#ªL?t}Ô8??Fl·0·?XÊåö§?r&¶Oî6ø?p&ÒEðm?ï4¡lÕ?¼³B¸v?v "*Ù´È?|˜ËŽ?eŸ?"÷àïý%?‹®[ð4|?ïóöüe«?=8îY|__?3TVßÈ/?W™JM©?SNrBTpÀ?9€†tA?ïóqÓƪä?VȚMʔ]?Bɸî†A¯?@Û8Û??On÷öÎ03?Rs´!Ĺ?ï|T¸Ã^?r{8(½?XÑøŽ§79?i¨cÁ´€?Ð'ëYÉ®?çÁ+<?î¯KQY†Q?—z·´ÀD1?€Së´ùWS?€`!õ¾sœ? öOþË ?"²žÓ^D+?ïÓŒ®?d~‹"i֘?Rr îŽô¾?EoŽ˜w³?qánç/?axL†´gAGN4FGL J2136.2-0642¿í¬búK53ÀC¼ƒÛÂ3À:çž?ñˆÀ<l*YoÞ@bâ'']@6¹£$]?Ä%W'"(n¿ppëGÀF@ÃÀ0²$?ïÿ*þ~ð¿é$žoí#¿âŸŠÿøÉ*¿ìCžOá¿£¿Ïg¿Asè°¿ïÿüñýAGNbcuTXS 2133-069?ﱊXLâ?{)v,íGæ?Fâ-Ña?@>lÉBÌ?'Uÿ8Ie?z;_nA[?£ü7ã?ˆVÁòm	2?^T³¶ÓG¯?f<~N¥*£?†Ê@'¦Â2?"⣚Ĩ?îŒLž-ý?•$ò¶gñÜ?tú±ª¼"?x6÷}Åfž?¤›ßçS-F?"x@¬¹)?ïžlõvº?e?{YZ¤?E[Cîpœ}?4
rMA«?‡`¡ó‰?dx¶xä£?ïDmÜì?˜¯¸ 	¹&?Z$Hf¥–G?YˆM)?šõ-¶hÿ•?˜:¦O˜,?ïRchôÐ?™uc'´v?`U
Så?j¨H?›Pç-‰?—Æok·
?í-ü¶…žÌ? ¾¶àV‹`?'VÆN-?€6
Q¥û¯?´Oït2%? (O¯‰©?î¾Ù)Qˆ?"úànZÊ©?aC?֓Ð?Uɒ÷¼).?£3þkH?"CÀò='AGN4FGL J2136.5+4259?Ë@æ碈xÀ:î}÷|¤À9Ê3°0´ÔÀ;´SFÎñj@RŖøƒ@Z—ÆZÂÄ?À† •÷£?š¦ÚtÖÌ?×vC=ÂXU@՞ñGU¿Öܱ±¾S¿äÁ/	ØÆÖ¿é`›š›ø¿á;4‰tˆh¿ïÿûB«÷¿ïX—;ˆBAGNbcuTXS 2134+428?ïƪ‹{Á?®"ýiˆÂ?q.ª—§'?®"k›$KH?fù5Rsá?bÜrH?î÷æãÆ°Ë?¦–`
Iš?4}#&'Kè?HB˳íf? X—~ˆÝd?¦oôÏr?î¹ÒQF¾?•|´ÿ÷S?ÐYÁ‰Å?€Ìh^p? hϯýŸƒ?'¬²Žª?ïì5Ÿìfh?E
rÏa'
?%G§€ì¡?J¸nÅ?buåj""?DK›:n*a?ï×د8D?l4ÑØu-œ?K>Ð8Ò|?Gå%ÕÅÎ?p«æz¬DE?i{"—¬†?ì"WÛu\?½ÚûV´(?NvK^F'Ù?geã-?»(VúýP'?½¯¨Ï—'?íàdªè?(œP´?‰Ëƒ5NøS?†ÚÊ~x\Ü?«…(êÍ]?™[DÁf$?ïÊ"V	?c¡—h‰¥´?@ÀV©ô?1ïàì$ñÑ?xÙ²üP¤Ü?bŠpÜ©AGN4FGL J2137.4-3209?ÅOQµ2ÀGób¯È°À;0vŒNW|À<®Úb·…=@ _Nã<û´?û0"|Ñâ¶?Òy˜\؞?Ìç±"_É?ýÚu+ü@—2[%@¿ïÿß´0Õ?ïüÉ_o¿ÖC™J~(¿ÖÜL|Z¿âi[
lпíýZ~{°ûAGNbcuNVSS J213726-320755?ïé§;BÌ-?QofÊwM?7v/z?^?$°wíõ¤?ciþñÂ
‹?P(ªbgã1?ïÐ-šË{r?s³ñÞx÷†?EB`ÖHÎñ?LƒùǂÍÄ?u@æ|"¶?qw汜e?ïuà¸Öº?|H
¸š*®?f!ÏúNô.?lÆÎøumý?5"ȏÊe?x{)
äÈÙ?ïek¨Û½?i̇ìi¾i?]³æœ¹?@Åz?Õ¥?'€ãaáÇ?h«IRÚòm?ïØþH'7?_û7	"m?J˜ÊÄíM?9àÖÙúo?p¨þœÀà?]·áQ™Y?ïsÐ`™â"?ïN{ôM?U92^s"'?aŠ‰@9?2`ÌßÇD?ŽPÐÞòl®?ïâ=Ä©	?†Ïó¬›»?lH§á՗?q[ˆW8?˜Ú£hê?"ßÜôãe?î©JØ|"Œ?'…®¬ƒ‡±?eŒ7~lþ?SÜȐ»"?¤9±',ð?'ÁQ©DAGN4FGL J2138.3+3556¿ïå3	†€QÀ(w°ËæÀ;hájéƒÀ<}~´;@ ß³î¯u¤?ü±*ÇC ?ÎØLÈ/¯?Á>Þwšj?î3ÓÃt^@î¹[«Í?î½cm¢¿ë±K1Vº!?í˜{Ò7ñ¿ãÞ¢ýñ\ú¿×·†^ÔKÇ¿Óu3=šiAGNbcuMG3 J213809+3553?ï¨I9§8
?v̔Þhêq?@ËHä{²z?1]Ü/ˆªf?"àüùs•?v\
þòÊô?îÃÔZ'#ÿ?¯Ô!Õ½·?e¤$Ö,Ö¥?€ß´b ·?¢hxÉ^3?­x^ƒÀ½?ïæÇí~?ˆ"ÜkP[?brüI+µî?g1ŽZ-Ãg?™ôÇs¹¹‰?‡¯ˆsø?î-Ê´LUø?Š'#Ö*
ï?_݊Ç ?R_û
â÷ž?¬*­ÑՍJ?‰¾wštá?ï%ý9®?Œã:Ü?U"±šŠ6ý?I=Yè1"™?™èãS.Î?Œ>~ß¼»?ìʋ9¸0?Àxpù$?pÚÕ/'"?€«ªÙT?¸øàzI_?ÀZ"LþW×?îz1N?™6ívHX?mh"£úãº?pš(îµL¢?­)­m?˜*ìÀ¶×?ë&ÐJJ?¦	üAÕD?j0‹ú¦Ð?gˆÑ8J¬?Âþñlê9?¦t4fVN«AGN4FGL J2138.8-2055?Ó¿6™ªÀFì¿Â"OÀ;6ÍòfºÀ<ŸK·Žw'@!N¦.Ð"?øî"ã)/¤?ÐÍ>aº…?ÊÓ=ª/"ì?ü)T!ÀD(@ªL›,¿æ¯˜Ÿá²¿ä™Dàá6¿æ9¨bŠ8Ô?½)6@j£¿æâ
·'$¿©Úó+0ZfAGNbll2FGL J2139.1-20541RXS J213852.9-205354?ïæppf«—?YÌ®t¡…?:5Õ¦~?*ñ¸ÓD4¾?fHÕw‰Å?W‡j>£ƒò?ï·i[ÁÐM?xêñT.i?PLõ²¨±m?Tó¾9rN?€
[{aW?uÏÜÀ@'Ž?ïa¥Þ3@?NïÜ,Jf?c÷ŽÄ_à?^ìW'>h]?'Ll%~Oø?}±©&E·4?ïÛ–Ä?{ÛVO²c?]¦1ÐÛå?LG"£Q3?›ê:Sµu?z>jÅUë?ïË3áj#ñ?qR[gû~?J¹<èÓ&ë?B¶S›.P?w睊IW?o\¦‡a ?ï=Û¸´"?"ó˜P‰ÔV?_çûuY,?g,Ù'P2?–a2'&ó/?"øÃ_a?ï:o+v?‡E…ĺ*?fî»qŸi?]Þ·øE?›Àa:Ÿ¼ˆ?†Y@ü"?íNžu:X…?—¶aKU†?pâW×*?dá6aå?´|æåL¬s?—s£3øà9AGN4FGL J2139.2-2214¿ïÎÁ»îûmÀG+'·þÀ:½-Œ*EÀ<f'}keª@ÎuÉ/ß@Ӛa?µø?ÀÉp·M3º¿²¢Øü0?ÙeèðïÂ@çØŽZ ?Èòdvw*¯¿ì=èîÁ¿à_$ù´Œ¿åœí ªD¿ïøÊ¿˜‡¿ïÿþ½à ¿AGNbcuPMN J2139-2213?ï¸Tv¾'?sìÄÅ/Š2?brÅh)2?\JÈ%H8ÿ?zœbNŠš?pñ꬗…?ï'×
?"žo7š?bšŽŽ‡?g(,⾩?†Ôf¬ÙÓ¡?€cŸcgke?î»XU×w÷?'tÃÃҍ?ˆp•
àûû?ˆ ­s»ðy?œ\ªºy9?W¨LS¯n?ï/cìtÄ?vøùÙNÖ?pâÖ|‹…G?XÊû\jç?•ÚÌÙ{˗?t'ͬë?ï.
©É‰ï?•
Úo9Ù?€o"^ªH~?xƒÍW2Ø?'蔍òñ?'ŒNÛÄÝ ?î̞cËh?¤Ïú!ñKÅ?p·['ø°?zäõŒÛWl?¡3H˜$n?£‡"gO?î
U _JW?˜·'´ðM‹?ŠµÉÑÕ&?‰,<ÉßÝv?¨­F??•.Â3Œa‡?í´nPâèå?"Y Gm.?ˆnQCôÎ?z#aÑM²]?®† .
x?'9k$žíWAGN4FGL J2139.4-4235?ïƒ^+¯[MÀH*løQÀ7¤P«>¡À;=€Íù¦@ǘ°eŽ?þÞº))?•="½5øW?©(÷"¿P@@#L]¦¤D@Æu)LÕq?¹³V.4ñ¤¿Û:ð@ð¿àÈÎ:‹I¿Ýó§ªS¿än'?ßéà¿áyÑÕëYAGNbll3FGL J2139.4-4235MH 2136-428?ïóê<Áž¾?HŸ‰¥ø?+qøT­—? ـ߱Ã?T½GìLGÃ?FPƒ]µ»x?ïã
š—?lË k×æ?67x"y‹'?Bª¼ól?j.÷`ˆy¶?jšØÊ68"?ï¦zî]Á&?'N3'Ÿ™?fÔBáÞ?vzxlz^	?€¬>§ýÞ?}oÏïÓ?ïóö!ã];?@¢HÙêj?=gØ×Ï?6ÁØÔbì?Vßå‹9z?@4y‡¿ø4?ïçÔý•9?[a¿"&?/‰m
f¦?"ZÒp™Ý¡?f2k¾9>?Z<RßÕví?ï¼±{LÛ?œó6 T?J:ãȓ4?`ӎ³8³o?~` E׏ó?€yµ'†ƒ?ï£Bœª®?…±µì¡Ùx?buüF8#Ø?r#ù©Ù""?''ÙՕx?ƒ)Ò;ø?ï맮kt?Tÿ5…íó?þAp‹Ö²?Ebn|y?cöf`s"?TƟ&€lAGN4FGL J2139.9+3910?ç5büŠ»ÁÀ$$ƒDÃ~À:^íLŸÀ;íGô‹W·@ܹ©.@¦ÜG©ã?ÍþAŽë–?¥äìź?׌4á߯@‡P&3¿ËŽ²µÊQÈ¿â÷Lg·Ÿ>¿ëõTáä·¿â?°"—©Õ¿ï÷d?ð…å?ïƒ/ÊÈæŽAGNbcu3FGL J2139.5+3919B2 2138+38?í˜á±O2?¿""N¤[?n}}Æ?xu›5š¨?²K_Ê°?¾'òŽÛÙ
?íQ?´‰?¼;2gþŽ]?e°žÿ™,©?wc|eÑ÷÷?¶‡ñE~Q?»O'–H‰å?í†fp™½x? aRŽêÉ?†=u¦ÇÁ?…•KRÐ?±*jÅmH?žò‰¨h?ïÄ='?bïd1nì)?DÇµLV?03ëÑéÙ¸?{ZÿØûGÌ?aÔlU2(?ì‹er[ÎC?½4¾'f8]?o§G‰VØ`?q¦;i"?º§š4zŸ?¼¦ŠƒQ-Å?é¿|aûG´?Çm]¹Í_?lh0Ûµý?oU}~é'?Ȑm´AW?ÇF-8å?êŽ
ϺN?ª¿qò^ò?–{	vüT³?ÔUÈ­…?ÂøvQs˜²?¨æ-f­˜†?ïF<Ð?óá?"3¤Œ¯­Ú?\°³Þ1­±?O¦3ç¦?•mZµþá?ƒzî!­AGN4FGL J2140.5-6731¿Ö€#¼ÈžÀDGë¿×À;&¸Lã¢À<ߺmN·ô@Z=~»œÏ@8ÇAr'?Ô2È?ïí8Go*Z@%žÀJ‹@uçâQï6?ïØB¡»&¿­}õ¤1x¿í…B>éÊ´¿ítÈ~ßY¿ïü•è41`¿ánß{ûùáAGNbcu1FGL J2140.8-6743PMN J2139-6732?ï0äQ¬M¯?§g¯š??{£	!ï@y?ˆr"¾87é?'ú³‡MÞý?¢é7bS?ë1³ÓpnÂ?ÁxŠå:›¡?µèEá!Ï?¹²ëÜÿÂ:?°Š'íy£?©wÒx~?êYðŽj]ä?®]¶'‡?³þP8¸¿`?¤.¬õBÂ?¹2+SôQ?¥ÝSÙvu?ì·?F£?žùX_×Då?µ!ª¡^?›ÅoÜc?"•mšJ4%?ƒ†G¥ò?îh]*8ÉÜ?°´ß#\=¨?‡Ð)+Pz?‹ÉÛ×Ù?£†#§!?®=Ӑ¯g?ã­éÑâ?Í敩R§Ë?ÍÝF +Ð?ÉÖ½àåwW?Ãk ©?¹	¦PT?è/uëáÝM?³iĉš8Ÿ?ºŸDօ?ª±¹Š¡?ÂXÄV‹?®‰-Œê¯?ãfôËeæÜ?¼.nþ:ƒ	?ÔíV+t'?¼#ÐûÁ¾?±äL"öÙ? ‡Ã<jAGN4FGL J2141.4+2947?托Kª')À1/pyåŸ,À;»Üº€šÀ<u<;±'@u¦Vkq"@d˜Þˆ¶ó?Әíùþ?цÑ`/j§?úûs5X§@µ‡¼!ƒÞ?ëQóþ¿Úž+Cû'm¿Óä/à'S¿ç\cáPè¿á÷‹òç鉿ïÿïÕAGNbll87GB 213913.0+293303?ïÃ2YÄl?o•çP+F?P0¸5'Þ?@‹Ê<™Û?zZ¥µÿÓ?mC:Âg¦Õ?裏`‹¶?g8(|9?]a/="?bí';ÕW"?'jƒHž¦?~7Qò"K?ïZqKØ×®?ùÞw?p
¦?q'ãÍYb?­øDÁ?TÙïr°¡?ï͒D'?r"¼3r¬D?g˜]åOƒÙ?Iˆ²nÀø?š*zŽ!Òt?q}Ö!?ïunKq?ƒNÒÍú?a¯%Å,Š?T>L:nýk?ŽT$jNš›?ƒ.ié?ïvO#)? v3¦Hõ?s{Tû~Þ?"Þ!P56>?šrhóÌzs?š°Ñ¿[è7?îÙð8""[?¯¾-©"¿?y²ŒWô0?zƒç›z-d?žUUåRŽ?‹TÙ}-ä?í}aÀxi?].hÏön?uXãVG$?e‹žHÕ-?²¿ppdóÉ?-¹1q‰AGN4FGL J2141.7-6410¿Ô€˜_÷{;ÀE#KßÒcÀ8;"‹›˜À;ÂûB+»@Ðڌþ×@ÞbV6mz?œ5Qßµ?ºIؼKV@Z…‡"ݘ@ÇùZ"z?Üŝƒ‰¿Ýïâ+XÉ¿åwŠ~Ÿ¿äø¸BÒ¨¿éKʾՓE¿îˆŸ@¢‡AGNbcu3FGL J2141.6-6412PMN J2141-6411?ïփ0ê?iŗ²b`?Q†1mÅZ/?O›¥Šœt°?p\Û¤‰=R?emS9Á?ïÙøŠÑæÎ?tÁ™®`|Í?<=ڝ?Jq•©¡[?q?ÝÄ+?rßmPté_?ï˜ß^'?ˆ1h}ñ?g*e. ?t}"l®!?"..âL®?†<×÷*?ïø¡g¡Ø?6žd £æ˜?&iÿ†?#{Bƒ?JZ7â¬Ô-?3ûôj†?ï•þ8C'%?'烲²†?W¼½Þ*?V& Æ·?‡ˆñŸ¢Ä§?—ǹ'àN?\Ššx?Œ"^±o?[{2U.±÷?"dkhô€?ƒ®B£1«›?ƒÎzm¢¤?ïM\zæaZ?'™dDÂ	¢?qýçé,-?|ïòfCfÁ?'Ôö­j»?J"Je®ú?ïì&CXÛ?T"¿ÐäC?;
a2æ š?0ÄŒ
W›?`xp¾Qßo?Rpº4g8eAGN4FGL J2141.8-3727?ï"öªõ?:ÀH‰GyBÀ9¢âž43À<F!*òó@9f­6Z@ÞÚ4"\?±Ë¾.ú>u?šwA] ø'?å	Ö¾IÚ@#ƒÊÐH¿Ö*¸¾«¢¿æá_¿æϋXŽ6¿édk"³Xˆ¿èt·,Q—¢¿ðAGNfsrq3FGL J2141.7-3734PKS 2138-377?ïûxÈNôì?5T®"#Õ?ÙGºY<'?¸zÑ8?=ƒk;3xØ?2òYŒ¤?ïçJ¾ƒøŒ?tØ'S~n?4óùx!ß?N"\LáÌå?fÂ2ÌY?qŠ‰¨­*=?ﲀ©ÄÆ)?r–"\_Ã/?U=¦–)?DÉÓy^m£?€¸ Ä£äó?r=¦ÖMg?ïò£ÿVÀ?=¢¤Xa}?:mïç†^Z?#pÖíͶ?U=<…œ(–?8†1,û6?ïô>-+ø?V=C?/'þŒ‹?.$|œ		?S¢ŸnD'4?SU¤âÎòç?ï¹ÊºV†'?÷•¡(?AyŒ$x:?QÓôJsxi?€u¸¹¦q?€ÔhúÇ?ïaPIeñï?…#.4D ?bKã(éä!?_¥úñSç?'Œzn¨v¤?";0Æ•?ïÝÌäA*?\͈0~­?QÁáéÁވ?CI¨¯–\o?iR*ËTÚ|?W²!Õ,·­AGN4FGL J2142.1+4501¿î_7I²ÀØ×à&EåÀ;	r£‹‹À<|CécÜ@ תU(¦g?úÒéF€?Ò¸D‹ÑZ?Ѿ ™'¯?û'fŸqJ@Þ«T4¿ïר¦Ó?ïû@Ô磿åʧ=Ç
쿼Gmý´¿ãCcaÏ'ñ¿ãтÿyGjAGNbcuB3 2140+447?îùqXe?•<ë;úam?V³á™ºˆ?G
C½Ÿ¡~?Ÿs^\ÜÃÉ?"æÂTs¬?é®â<[â?¿ÓÎ/½O?a%²;Xö?iÄ'¡ã?ÈÿàDÁ?¿2g±?(?í¶ý/ô—ö?›ãê¥Ä­ì?{|ö˜qª(?và¾
Mé?°Gcp?šjÞO"z?î¡¢iÌÍN?X.žË?s'Lç~?WþZù	¨?£ué.y?}'S¶o@?í•/ò-{Ü?§ƒÊÛsM?g–eö<§b?X—ϝX¶?²™Í>^Jé?§L-àÕt?áÝÒәg?Çïgû֔f?s÷ñ¢vè?‹;ݞ"·²?Ûôz'å—Á?ǯïáêt?êŽçb?¨ü¤½Ð_È?…ñã•b¾–?{Ì=W«?ÄeE|êiô?¨4I<AÌ??ì±=­¾c?•€n<ƒú?' …Ï7…?s3ÎG ÿî?¸2îSõ?"ŸÃ
ÓAGN4FGL J2142.4+3659¿Óáe…ÀÉ´À(Ïå†6À:x(E™gEÀ<Rñ¹_ä@ Äbr'æ?ÿ5Hyd?À]ÚPÃè?"/Àô½å?Ê@±ád"@»ti3uM¿éçkÅ?ïýTõ$Ú«¿êí¢ò(§¿ÌžnÀ}¿Ø`ÈðŸ:¿ä2jGâAGNbcu2MASS J21422658+3659481?í*vH9]?ºmPŒ¼*?tdü­‡Ü‡?x—…HI0?µi4"¾‹?¹Æí²W?ïÚÏU#"%?~¢é"ÒG?/ß<"ê®8?<$r®Ê?q™[§4ӗ?}ÝçÜÆá?îî¬w†Ž?Ýiú…ò½?hçX+¶?mgրc=k?Ÿ
Ž§ÛÎ3?Ž)À–ÿ"š?ï"zLTö?f4°‰ÏÙ?]ZƒlVÎ?B·cQ†¡ï?‹Lߏn³Â?fu€"˜ä?íOÖkuޘ?²O-"`l?~ir€C€?ŽhßwªH?³šµ{ˆ?±kcà«û?ïl«0è!´?¤1ì兦)?E"¶±ªùé?Và'ŽLÞO?'Á",:"¨?¤
½x4ß?íxù/E+È?ŸÚ¶r×Þ°?vP¹tŒ	/?u§ùŸ6é+?²Ó*ð$²ë?ž$ð£ŒN½?î»È%Eá?ƒ·£ñ
€;?t]ÛWõú^?aÓ¯Ž$OÓ?¡·Â?ÿ?(?ƒ
USȗÇAGN4FGL J2142.5-2552¿±m'ŸS@ÀGý–áXuÀ:h˛teÀ<nÉìG¼W@ªü~ìC@Çùä]K?½Ùz|rí?À=
w}:@
;ƒcÍ@ãÃ"´?æ'ú㱿×Pâp£K¿çV±v/¿Ö}ê;ž¿ìÑý"ÕíÞ¿ï¥è\uKÜAGNbcu3FGL J2142.2-2546PMN J2142-2551?ïÞl^·?cç‹ì³6?F
çÆÁÒ?>ù[
û0Ê?l¨X p?a³Ïßֆ¶?ïã™
±?qXÔq¢ªÈ?:¯Ï'ÊyÎ?K<"çú?i©méá…?m¶¶¤'¤?ïÍF*—ê?"½þ$tÐ?saˆTN–#?{¶i|§
½?'[êOª8S?|¼¡‹Gr¹?ïÖÿJùM‰?O˜ŸºæS¨?P瑛´¬?5ÃBé>\"?pFv$« L?JzX†D‡ë?ᅪÅ-¤²?p$2ªnHs?]7¸×a 7?SÙR9j?xë/0•¯4?jÚ:1 Õ,?ïªvíXn½?‡Æµá—ÂÑ?K—')Æ?Z»`´¨ò?ƒ°ë'PZò?†'Î͙U›?ïeïÕC?‹ý͙<?uÖK|±P¢?€¤ìaÔ7¦?‹°ÞQ&Ä?"<ÄßG®?/–Ø?kn'R¡Ö´?eÄ[Pëû?Sájki<¨?ƒ´ç"my?f"7=*ÚAGN4FGL J2142.7-0437?é}y'èûWÀCä"&þrÀ:¿)h¯À<ẕ@tÀ‡o@ö‹AèÜ?ÈÛÁœÂîÓ?§®šÑÖL?ß¡/$°¹q@ÍåûŠ¿ã:;e0ÜA¿ã¤ñ@õh¢¿åõ²Ÿ$¿á%sW±N¿æ¨ Åó?¿ðAGNfsrqPKS 2140-048?ïˆfŸ'wû?£G–Žï"ï?S£ ˆ?gV£¦¿?‹qõ2>
#?¡ò0+éSE?ïÁ¥]¶Ù4?uÛď!'»?HŒ…6(IG?Ož¥Èñv?|À|9½ã?sŠÃð\­V?ï~å•Ö?r
ŸðèŒN?bǤ‰Ú?^¯JŠW§E?‹õˆT,?oo QŠ³a?ï'È1\™^?c<¡Gà ?Z]T0Ì?:âˆÇÄ°X?ˆ
Gû˜òh?bž§:	Ù?ïl2
>?˜4Lˆ¥Èª?[Þy6':?a"/'ûé?ÁR2aX?–n/·²2?ïK"Y,}H?/Z—˜eý?Yäþ»h­?e¨SÔ¼þ?"ýdé:v?[Ç#4?ï$2cC`?€,vȼõ?jþ62Y?dŸ©äÏ|Ç?˜ìÏÇ_?}QMËõíD?îãíñh@9?€ŸŽñ?m¨2ìÂݟ?Y˜¢!I?ŸÍ;mÐy;?€&¤"¢|AGN4FGL J2142.8+1958¿¯‡3p²ÕÀ8c`9%»{À;°)(vÀ<ŠxËøQ@!q¹7C¹?ù_=?%°?х™ž!?ÈA÷[ÁœÃ?ù®} ½ê@	XfŽTl?渘B+ž"¿ì%ôïo¿ÄÝ·*Ï¿ÍØçø¢=­¿â?`A^D¿Ê4³{mÂAGNbcu3FGL J2142.7+1957NVSS J214247+195810?ïîàÉaò?Yäq‹µäª?'úìÁâaó?"&›(|V?_?d•ä€?XAo6a?ï¿îß遆?y=?Ck?LUL2_Ó7?T%à‡ ?|}æd•WH?v¿4)C˜v?ïs¨W¼CW?†Nä§z{ô?R1qŝ·?SžTqö?i!ï£mV?††[ôÿc?ïHNEæǨ?pàqԋ?H{'Ržá?.¯`ʚ?–2^ž‡DK?oނ+é½É?ï݆¯öÂ?m+É:Ó±à?7…ÇAn_ø?1Ô&qÿ'Ê?oˆ— íF?kÔÁZè*?ïb
¦fd?Že;
à"?TëpŒg$z?a,äRcæ?'o˜ÆX+?ŒlŒGž?îîëv
Öá?'çì-¨>T?U€J2<4?Pt·ÉmºH? eFL\ÓT?'Ø*VžOê?íåÁ~ÿ©?Ž­¯Š£…Ì?W°"µ"®ò?K©[tÔ§—?°y¡s¨z?Ž˜!'
GAGN4FGL J2143.0-5501?ã0û»LǯÀGh3Æ*À:·"òsOƒÀ<lꭈcç@jŠbo@…ËÀ]?Õ¦"»ë?ïÿšr¦ç@Ĉ'ðà¨@gIh~¿³Åüà!#¢¿æ¦²¡¨[Ô¿ïþdõM—?ïp¥ïé1‡¿ïÿìIiÖ]?ïŽéõÒAGNbcuCTS 0561	?íMûÀ?Àã[Ï´ˆ³?´v˜ÈT–?À9ðÜÌt7?ˆ7ºûjÏ??šúV(óÃ?ë¿^y ìù?Î&ÖήN]?ºݸ¼¬?Ëz…ná¬z?Ÿ¨º.t?¢öRf±
I?êÜ­åxa³?«ˆ£CÂm?¬?óO·[? +Ú,êkZ?ºú—(ƒµ_?¦|£(^yû?ïEfgÉã?—ç×	ÿ—¬?'™o;òÖi?–é «Ì@?vçgRÔÌ?r4QXp?ì3ÌѪ?ÆëQݘL?½•Š°Å?Æþ°Û»¹:?Ææu¿c?,ÃÚEù?æ«zÙ Sn?ÔÓyq'ñ?ʞ¢R?ÒùXH
?µfå)âgï?¶I^Ýá?é)÷s¥¥R?­÷ÆHïË?±ÌçvÊ¡I?¡ÉîB"Ï?Âq®v©S?©$œ1æ ?é?ÏB×é?Ì¥àS+:?ÈÔÎÆC"?ÍDÙä7w'?—qF›??›D¤?šAGN4FGL J2143.1-3929¿ïH}'róÀH¢ÛߏG0À9õƒ.I½À<W"4$Ê»@´çër@(¯œ:]Ê?´F¾?ì)4¿xÁ—©CJ?Ÿ±m@ôÙjM?ë.Áÿ"JO¿ÛWUý7£°¿åJàc'†X¿á'K3Úøß¿æ!ú[{PÙ¿ÌËc@A8¯AGNbll3FGL J2143.1-3928PMN J2143-3929?ïõ$â¸qv?BÛó8òØ?$|3p åv?õèÔ´?S&´¤&ÛJ?AkÒù¾½?ïéãDC·÷?kf´I³$H?,•ËØÎ??À'}3³â?dP' ö??i=PÌPo?ï½ð+oð?i¢9Ã˒?S1¨ÿF&j?Yoœ?|;‰š¨JR?fzuPî[?ïåό½	®?HùÞæ®û?3Ÿ—l´Ož?ƒ©Ӕ€?g¼€(û;?HÀð "?ïê ª&|
?UΠÔô?4ôc^&N?"cšs•†¥?bۗƒ¨`C?TnÅÜâó?ï¸mÁ£à?'¨ÿM¡ê?=n9üËw?Kž»÷O	?€ùHJÛg8?×ÖK<ȕ?(¤¹Þ?{§xö¨Ä?\k[L
Àú?YÃzµF'?ŠŠÊb©c?yÃC¨øB?ï¹1¯¥t™?fEUåÔn?J4Élm‹?5?¥*Á?€Kþ4f£?e&ò}ÎqoAGN4FGL J2143.5+1743¿ï«"õ´¼OÀ:غ@ÙÀ7gþR€ÖTÀ;iÍ9VÍ@ù§>Ê@šz…\!?5…¦{2?£gQ×kâ@
…bÅÇõÍ@^'Š]'¿Ñ±U¢ô·"¿äâaÿÏY¿çRºýÂc¿åÉVAU¿è}ÿºà¼¿èÌ{n5gÁAGNfsrq3FGL J2143.5+1744OX 169?ïõkíÂnX?G׊§q"?1b˜q?/A	aK?PϞÝR
w?DRZ¯Ç‹?ï®Ç
p+?'9u ÊÊ?VãJÝßǹ?t A¹?qÓ<2¢H?‹Ôœ±c˜?ïo˜á…8?"á^í/ʜ?'dÁ'T'?†É²¯øÓ&?"ÎZŠrÜ­?`¥1R]p?ïéPˆñ?MÞÀÖy'Ì?Eÿ-<ZcÆ?5"øúØ
?azäh›#?HÕ5ÏõÑ°?ïä0/Œyd?hv¥$ôum?8—M=Å"?3«c搃?h¼æÞ~}?g§\õ'J¤?ïAâÝý™?§EEÚTʳ?`õ'7fš?v|h´¬À?•¤ÿU—W?¦¾¦·lñÎ?îÒsv*Ý?—íö§·u•?†äåk€áÐ?‹Ñd1-?š?}÷…?"{BîŽí?ïÍÎË2KŠ?lv⯕ÿ?Z…öÙv€?Wm"
ù?rw'¦?fXÜõÂÅAGN4FGL J2143.9+3337¿æ_–éfÀ-s¡ƒrçÀ:ÆXaÀå8À<iï¤h)µ@ aê»PR?ÿÑ*)Ÿ6?ÃZ°ûŠûF?«*n­+È?êpå^"
?ý¬ó@T¿ïù¥þÐ¥?ïÿû˜'2¿¤ÉlßÁ
¿ä²¥~Õ(¿áy‹X࿼ÚÝܔ•úAGNbcuMG3 J214351+3337?ïÕ¬â0?gel"xKF?Ahp˜ªt?2D˜XËÿ?sT|`¦€?f§[Vnrä?ï³,
ÎÀ?ƒ"1 4#?RŽt‹ô?Z:Ê:{û?€ã.3R;"?'ÅdŽK
?ï'­ ½˜Z?¨zY£ºy?vׄSfÐ^?'ÓzÛÒDú?•TzÑc|«?‰0ÊÜ?ƒ?î`²ÙB?<œxO&Ä?xëhûãVú?_ʨjIÏ?¦á*ǑÀ?€c>†öl?ï´(X¹ª†?vT\Q#Y?U{ƒKšw?MBÙ'®i?€Fˆ8<ï4?u!·Ê®þ?ï#2Æ7ª?¡"­0û›?eË]'
[?r‰ ¹±E?˜à;™¨? óÔ]Øû?îҋ»_'?ŽˆÓ¬Bœ:?t††7)F|?wG`ò $Z? Fs"kñ?‹?…—}6?ìÅkÚn¡?šóOðªÏ?ˆ‰kIIÄ?wµwtlj¸?¼0§8yÕ??šÚ{`ƒAGN4FGL J2144.2+3132?ãjºŽå>;À0M>Õ'å!À9§<t$•À<+ºõ3ô#@S0 U @ƒ¼ûžqp?³êoJ×?­Y2Ý^%¶?ø"c¯ÒÁ@
<'A¹2ç?ïË}ÂM—ã¿ßAݨ[S¿àá–5df¿ãªŠLõ|¿Ùʊ<ÚPï¿ê) ¡`7AGNbll3FGL J2144.2+3132MG3 J214415+3132?ïðÆjnD?P?ñ8֓j?,Uc'wbÅ?W2*šik?Zè~h——W?NŒäƒèwa?ïæ:x3â?p¨_{)Þ?6ï¥.±ˆX?DKßZâ??f瓗ŠíM?m
Wn¿6õ?ï³$£+j?v*‹¥(X»?Z¡Öl\;?e[zÕ=?Å8̬ÃÑ?r8'•Ø'*?ï—²‹Ë?aÑÈ÷¸ƒI?a‹¡"*º?@s©¡7´?…Ú0k5`¾?`€ÎTbä?ïæ-}DW?[.@ª÷W?>CÚm%Y?-Sö"
¬?f'WÆÉ?Y¶ÔÞ)D?ï¸$G™,ó?ƒ!&NÉëµ?Hl8Åi©?Užk÷Þ?€p*˜+›¿?ô"+Äîù?ï~A{Wö?€FA}¯Ëc?czç̈Qn?e«pñ¥?‹çFà4?~,Yë§Û?îîw 6Åÿ?~í³}V?uQQjü"=?]êí¶?œÜǤkp?|ùÌHªYAGN4FGL J2144.3-7802?ê9†^m7ÀAuäõ8&À:l&ûíLÀ<£u»n@ôí}F}@C…%nN'?ÓÀ£~tÐ?ÐM`…ü¯?ödŽTÁù4@
3Ï.Pö=¿äþ÷Väd¿åv…}'âž¿ì"+
oÆ¿ïüë"£C?ïÂ}h‹…¿ïŝù¥žAGNfsrqPKS 2141-781?ïñ=šó¿^?~pv>Y…?HU«¦2"?pmxÌk
J?QYô9	£M?lëUá,"?ï»zçŸ-z?­ñœ8P?V÷CÒ=~)?pâˆyµ‰?|"»'<;¼?ˆèò±Þ•ê?í¸¡æÃ? d"¾K?ƒdìʶJ"?…7g[•
T?¯œ´Mœbn?žÉ‡=¹ƒv?ïöC ‹Ì?G!©'!ÀK>êIˆò§Ò>íÛb¤®î`?SD+½ðÔP?FûU·Ñt¥?ïòÉEP8Ÿ?[y²;ۇ(?H"çÕ­¨Í?Mÿ¨ ôD?LGÚõ'?Q=
BÛâ1?ï4VïÙtÙ?ªO›Õ¦=¬?eRe—¥HÝ?€ný°
Çt?–ÊÕW´­?§Ûý1 ?ìž$¤\|?¥›ÿ@æšÁ?%ÿJ÷G?I҅>/ö?·*=
û·?¤۝¯…?ïÜb)stt?j}§$æw?~á§^x?ˆEÿ;Ï7?qïðõs?jN»ÃÙ AGN4FGL J2144.8-1817¿ï¢Ð£WCÅÀG)ayWÀ;h¥IÑjÀ<ºqÊG·O@ ä²hG'?ÿaueݪ?Ì r}ËÞ?uH¥qzQç?¼ßŸb±P@vO[‡æ¿ïýQßñ—²?ïÿÔÌuŽø¿â
Ò¡"$¿æ¢f&¥†7¿µtSäوó¿â¿ý¡UûŠAGNbcuNVSS J214442-181801?ïÔÕH¶?qç¨ô•
¥?69ô¢ñeG?+jtÄ´$?t1¼<)¶?qr"7/'¥?ïÍU$I¶?vr(ÆX£Š?C±åºâC?NéD¡ ?w˜Æ¥Z?sîÁ7oe?ï
•åÚå¿?‹1ûYŸ{?eN§<[6?oB:Þ0v?œn_ß,¯?Š`$Ê¢Â?不*ÀŒ¼?kM $¦¾?;!ª—ŠmF?,g".dR~?…½(5f?kD€m®Á?酪^؟á?€Á¸§:éÎ?Mšsê™Å¾?DØkRîé?…wÄw?€3"R#Ä?ïÞõÌÓá?‹Ð-ž	?LÁ÷ÆÄ?Z½"¾ßV?¼1†ü,8?ŠSÍx‹M?î^n0›d†?"Ï*
H?pŒ4Þ±_?sÛ£ˆ'"?¨pŸÅñ?"8ÙMT?Ê?îêB䉵?‰¤Ø ™ÑÃ?N²wVÞâ.?GÄ¢"8"'? ãað¨!±?‰Æ=¢´½AGN4FGL J2145.0-3356?ÜÝNTºÀHÐGG"#À9HÆBoÀ<÷ïF4@֒­Â—@O,e¹˜=?©-ÝÞÂî}?¾&•Q¶@³w[0@»Õ]jo¿»v|3,RC¿Û–H¬A<
¿ãø#B$g¾¿æhH‰͟¿èÍÃØ1"Ý¿æ]THÏAGNfsrq3FGL J2144.9-3356PMN J2145-3357?ïã!O"?b\tµ]"6?NíÈßô"?H™ŒK™ ?e#vêBÙ?\f¬¸×`È?ïàÎKýÚa?vèƒ(íH¾?A<¨;?YÍy5šx?j퐑[%K?r
@ƒ"hÆ?ï¢t,³Î_?€
s#ø¨?j£b§‰V3?sÈdÎøø?€º3xæŽ?xÜFNXQ ?ïõs²ÝÀî?7:Mˆ¢w?'×^çÖ|¶?;9â_êl?R®¤‰/ì?4{:æñ­?ïªÂÎ'?zfWã¢?d•¯þu'?bFdôt(?€Y
*vÜ5?u%+Ôá@'?ï¸Á>=P?'b¨¸ÇÏ?RY!d Š?qBEÒ¡'×?	±)Þ?}ÎW0|kT?ïzíô‡c?†JÝ;2oº?qXñWI~«?z2× "Ð?ˆ˜
3›Ê?€¡r¨'Š?ïè|#D±>?Rb²MTҁ?9|+je­Í?+Kc>]o²?dTWLDL?P‰™qU­±AGN4FGL J2145.5+1006¿ïïÚ²#åIÀ?ŒÌxéö©À;^.†%HÀ<§Î_ª@!í9Y=?ûY'ÿ?А›ëÙ?·Š¼+R?êϔÈy€õ@.-%Òø`¿ïÿÆߢèM?ïì~Bûþ¿Úd\åX¿ÚÇýsޟ¿Í–ÿöÅě¿ßôâ?¥²AGNbll3FGL J2145.5+100787GB 214302.1+095227?ïξ—³n
?|_Ÿ¨Gv}?0—H"?þÎ?0ou¢ÿ&ò?w—?›ýA?{¨õ©N;L?ïрÚÊ«#?ràb"aˆé?@w‡Û€5ê?Mwnz$œ¿?u0¡ÀÔûÖ?pœ|ݪ?îφفÍ?–*¤³ö_?P'^!tu?W/Ò!?¢ƒtÓŒ?•ù­€D¹?ïŒñržƒ
?oÙSÒ:Î÷?<¢'íúß?(X{)TÏì?‹ÞAüϟ?o¬(šK?濾݆¼?†88±™?Ag!¡4H?D±;¸Øª´?…HVx5/ˆ?…DÉó#"²?ïwCü.9N?'rô¶˜$q?L¦OH	?`enf‰z©?2Mÿ%_?®ÒÜsmg?î%µl3?Ïçâ¼s?W»ú³,T?gÚÒú±]?¬ñäÏÆþâ?^áÅ~æ?î¦t+~'‰?‹ÞçsW–?L¾S…Š·?C=Ï)Eÿn?¥%ÃöôÅc?‹÷ÔË9rêAGN4FGL J2145.7+0718?èGӍJÃÀ@´Â	$lÀ:µmÖPÚÀ<]¸"Üû@ q›#òÎ@Ñ|^?Åçþ×`ú¿•vFáÄ^G?ÒoÞ_FaŽ?òH›—ËŽ3?ææ¼Aå'·¿ç^-¢¥†ã¿é_ωþœ¿Ñéy«½ˆŒ¿Üœ\AŸ\§¿ãh4ë~AGNbll3FGL J2145.7+0717MS 2143.4+0704?ï,hq³³?"#Ö"˂?TÕu^B'Ý?Pš`höcŸ?™%–¿)(?'‰¥¿ëÞ?ïflL¼·?ïüß?jgñÌЙ†?r	4 ˆX¤?Êð…Œçò?‹)8©+íK?ï&У"?ˆàñ¢
>T?ií‡,"˜V?kÊz0¡t6?—ÿ3?†þ5ù¬ÁÏ?ídd|g–?'ˆ"Àj4?"ÅZN¸?g=Ô2
H?²F©š÷\?íPÁ\­à?îHŸpj˜?¡<ÔöÖ¥X?iÌ{ô6+?bî¹*áY'?©äÌ0»KÕ? ¯³×ö[?î>x%«‹4?¦`œÍ¨?{ºÏ±e?ƒx†Ü»?¨¡#¯:HY?¤^'±˜ÊÚ?îUñ¡öèÞ?"B>Ž½í?sùë-Õå?sÎúp<\¶?¨!¨{œŸ?"
J"uY?è°êšÝM?§ß]|•¤X?œ¿
E]¹?Šx^ØÊÔG?ɤg"Yҕ?¨°J€ÄÆAGN4FGL J2146.4-1528?è·	'¼fÀFÑ|¯Ý©À:YyîÙgÀ<1£üÉêš@4I'n|à@Ì·ƒl?¿Î-_‰¨`?¿­0û›|?ø¥Èçdþ‡@ëɃl0«?ïó!3F¿ä½U¡E¿ëa¢ýpƒ¡¿é¡YìÛ`¿ëõ ޜØé¿ïÔ+{¯AGNfsrq3FGL J2146.7-1527PKS 2143-156?ïòké÷Ä·?Pqµý5öá?8p5tÕÓ?2bïåú3f?UöS?L±mÈ4B?ïÒ1¡@_Ÿ?sgtËß]?EûÜå]º3?Oa•ÓïA?t'³°>Ÿ??pÌ5*%?ï¬*»jyÆ?z¹Óõê?`$¡"Ón'?aÉ!
?€ì(Í®µ?xkqâI ?ïϩՕ·ü?R÷!iÇì?ZªÒÀÆs?>¨ƒb£¤?q€`fé/?NÛ®v˜å?ïæ?¾Ëœ?]1cñ0JF?LØ,j¯Õ?G}Œzìe?bŠ5ؼà•?W€ÛÒîä?ïm¹€?'‰ì ¦Èê?`í¦¶^‰?tžãʆÇ?\Ë.¨d,?Ž²ÐÕΆ¿?ï4˜Žß?'_š¼N»R?l²v…v¯?sÙ5µ÷LÃ?ˆ†SÊ5 |?{fqùíl?ïvÀ"2!?s]ÝÍGë?t\°ÎH0É?_#ú坫Ý?ˆ!¡5Ù]?n"&zxüAGN4FGL J2146.5-1344¿ï}†µU%»ÀFy—Ý÷wÀ8ë¼3øUÀ;‹Ûϟ$@Όïg+ˆ?÷ëŒ
dÝÐ?°y½!3+?Á±³ì{i@)4ÀÑìÇ@fûc
@…?ïGM1:Ç¿Ô[â¿Ó·'I%¿Ì¼&'j¿Ù"­‰'¿áœõ~DZ/AGNbll3FGL J2146.6-1344NVSS J214637-134359?îsäLž?Æáû+É¡8?¥"®Å%?Æþ°/ïB)?yhCŠ«?Q犲…Ø?ïc'B²N"?¨0bÈr@?f=ãW¬#?{C?w%Z?Çû>À©*?¦1
^vÿ?îcô):¿w?›ñôo@92?'¯aÊÒÏ?‰'!Rd?¥`"Ÿ[Z?™ îÐí=½?ìA:O8?žäÉ5!?tÐ	äv‰å?\™±L¾´?¾ õŒNe?ºe'jòË?îìŸ6ôU?°ð›'÷?‹£(E?®µuÉ)	?"ãJ‹Á+?œ>ºDJ?îtÌÈÆ?±.Ö;ˆ?RAÆñ?˜'É!æ?¤oãôE]?«Äa#žz0?îõÆJ}? ÷è»]=?‡†O·c´#?Šè M±Ç?©O"æ".?žpj"u&î?èáâÑ
?²¨¿c¿?'<TŠ¿?q'X‡C`?θºbú?²"èg
ÿhAGN4FGL J2146.8+0425¿ÏM"%™öÀAµB€®IÀ:—Ù
LïÀ<3ycՒ@ò¤ø`@E"FK=ì?ÈèÁà_¦¯?Â4õ«?ò¸M¹Ç7@¶Å4ý㛿萘~'€p¿}è(a·Ä¿ê@õ~丿ëd&ñ'9¿Ç=Xlþ†¿ïÿÿÊPËAGNbcuMG1 J214653+0427?ïâ6¶ e'?c¾;®¿_?Fi=-³œ?Gí:
?h.åOnË?`Ù^.u:•?ï¾é¯S¸?€¸˜#F–?OV÷WY+y?WR!TøKŸ?| IUnOt?}á,o-?îû_¦r‰Ï?ÔÆ¢Xˆ?}íΚÅM.?'ñٌ¦Ô"?™—…ÖÚ?ˆ–Äú†É|?ïÎQQ­ƒ?[.Z@?9³ë!ãwF?'ß]ðFQ?w;ù%Qe|?YÁÚ~YØÕ?ï¢VMƒZW?†œ÷0ÉW•?g÷•óNÆ'?tk'/q¿?l‡ƔÌ?X—UM?ï%çª4? êå%Yý?_!¦üÈ?pQÀÎz?™kÐì=Á²? ù#–Ü?í¤>Ûe?ž–
Ö­K?‡W'U¶Õ?‡¸e°¶?­ÿòLºÎ?› s[?ï_;"Qè?y\z95
Ž?Un…­?L<¾›KÛÇ?'Áº¥ ï
?xZ±šÚFAGN4FGL J2147.1+0931¿ï1LÂëÀ@×ÆûÒtÀ8h5qÑÔtÀ;Ò!¯}0­@'š¤†ˆ@u…zþ£ß?¡÷Hõ™L?¹"ö%j@t¥ß"9ç@h[J©q~¿Ï"ϝŒ˜T¿ãSßà›¿ç·|¯Ý©¿èØÍ÷o7Æ¿éd=ÔÌË¿èÈgÕÒ/AGNFSRQ3FGL J2147.2+0929PKS 2144+092?ïÓ®¶6]_?­ö=½Þn÷?I

¡Ö°›?AT%Ðg|D?sc7$´?­ûmÖ˜^?ïäÇ'ÏÛS?hhtt¥P'?8?ÁJIÕó?ESj…-Û?h0àA!Ÿ?eä®6Oðs?ª±ä?"Ç{uc+?l–ʧñ…›?wK¸pqn?"µb´y†?0(úè™}?ïøTïåi?36ƒà¥è?%-àT;[?äTDh'?I`Ìï]?0ÍbӐ׾?ï×ÞÎ8?'³£qcäd?Vè8	Ò?rýùï0(?mØ.
òzÆ?ŒÓã?ï´äԉa?'ááá£ÊÓ?P%±
™¬?a™
©Ú`?€ÅF7ž/1?¬¦"î±?ïD+Ø9×+?oYIàXL?qNÓžAg?{`oª4–?"&ÐWN?½£"Õ#%?ïìßö0""?SNnåöEj?<VËì—h%?2HgÁf‰?_*aÖ©È?PvqD:•qAGN4FGL J2147.3-7536¿²,õ®!ÎÍÀBDR½<6À7™I¬|À;Œ›aöK@ÅeÑÄ®@íüºÑ!Æ?"~<*©?±>uf3'@;8 ؽœ@²\L=Ý¿¹¦'ác^¿ã‡>ùºì¿æ18‡0
Š¿æM= t¿ê‹P*º¿¿éWòeÊAGNFSRQ3FGL J2147.3-7536PKS 2142-75?ïÑâwü2b?g»pxŸä5?P–"ëEÒ?D
Ëö}™?s^'aWª?e®å«GñK?ïÚ®Ø¬e?r±÷Ã4¹?@ôDŸ£¤¿?SYÁ—Ûm•?pŠ0œµ?Ù?p¾I-j»?ﵡÔjiÅ?©Ÿ
ˆ?h™ºQy2/?v:(ŸKTP?xâ8ƒ"'?yVIvJr?ïüÂÚõH[?$ø£‡¼N¼?UÄôã£?ÏñpÂÍ?5"¶Wï?"Ô2µú+?ïÀBNÈÔ´?qÂùõYõÉ?LI•Ä¸;å?Ba
NN?|U¥Â}ƒ°?pؽEñ%ó?E›@?Š 9l™l‰?Xd¶¢ŽÁÂ?puvtßyš?…,¹Ý¶óÕ?‡‹BÏï}7?´ —K?†ˆuw¾ò?pº‹–FŠ?{'(â²)?€Î5™ö#ô?€Êµî?ïøç'ÁÍ?C™$H¶û?%/Êõ×Øg?mÚPJº?J<oFF&?A~Ł^AGN4FGL J2148.0-0733¿ËãÛq5ÀE6€àe0À:S¡"I¦<À<j|>>ÿð@¤—»H?ý_ÂÞ6œ?Ä	Æ'l*¡?»JµA&!8?õ¶{ò¿¥@5˜þ")?ítM_.cÁ¿é§ ÉN=¿Ó +ïrC¿ÖH´å$‡t¿äú¬¤8Y
¿äÌqæÍAGNbllSDSS J214807.08-073347.0?ïϯ·û²?EÁN1T?=˜T¶©?IsKçükÎ?vN£˜ FC?s¬±4§
?ï®Lª¹¸¯?xÝCÊՅ¿?Twà:
Õ?U5Ù'n>?Ýñ—B`}?u÷Ix2?ïxƒáî¿]?uGÜz¤<ß?^ÿ°…á"?JÞÛ`~\?Ž§•¤u?sì ¨žÄ?îêfßÎ?pë\ⳃÆ?o#¾Šº¦?LÕúěÉ?žÎ¬SŽ%%?p"ÈÎïG?‡‹úõ?r‡(s'?P|'¨"?;ðó€UÂB?…KKû"—ý?q'Á¬é‹?ïöòÝz?ÿh(ÓöÇ?a~_Òޔ·?d,r™	"Ä?™ÑU§å'[?CmîÍ?îø"¢!ä'?‡lñ£?hƑŠ±"C?aA°7är"?Ö™"iêQ?†¦j0¢?í^¾L‰ùò?Š'uKUÐ?"€œTü?eq/S
óÐ?³åÔXc?‰eÔÃEAGN4FGL J2148.6+0652?äûc¯ì†ÀA™í|o½À9ñxKk8]À;ô÷Zï:@Q·&tU@BªA‡‰Í?²•>9x?ÎÃ핚0˜@jgÀ¹ï@
`ç\ðñÅ¿Ê-ªÞ•I¿åÖ]9–úƒ¿èºk5Øÿá¿ëƒï¾"OÙ¿ïÿúŒ—Ó?ÛÂð?˜œDAGNfsrq2FGL J2148.2+0659PKS 2145+06?ïòjÍ[ñ?L{CL»ÿ?HP|ígŽÏ??j5¡ð?O=×@l{?CbïäÏ"5?ï'$7V?‰·²ýþ?eá	»W¾à?u
/t¶ë?†Ct®¬«?"ºî'•?ï]kÙ?…žapšº?vóðt<'ý?uÄCf4y?+ŒÖxÙ?=Ím¬b?ïŸ]dlú?e)á¨ä?bI3§V®~?G41¹m?ƒ–Z0}ù?aãïþQ€?ïåÈGù?^Ƭs@?Vø¯ùQ?Pnސ•v?^jð>
	–?TO@t•?î—ôq	5;?§_((™û_?~œ–¶m>?ˆÜ-#4ô?¢­7`]p›?¤=	+à?îÆ[ˆU¾<?"t'ñô=?† <²0ÿ?…
~wîèÅ?›äpŸ¨»ñ?ÖT÷"º?îÂ÷¼9¬Ÿ?†ø…RÞËÝ?}˜¿AÝd±?jÑÿCóñé? lVÓ;ö?ƒßÊs]ÈAGN4FGL J2148.9-0121?áVÙƘÀC£2œ4~À;Ïëe>HÀ<YLÓi©@Z$×$êp@ºñ-À?Àî^—ååM¿µ"ÄÐÿâN?öÃBZ£‹?úäd¬R?îŽñ"%¿äCHT,§ÿ¿ìlü›Ç¿Ü¨¡õ2Ç¿Ö5²~íÆ¿°Bœ ¡O	AGNbcuPKS 2146-01?î*ãUÐA!?¿ŸÅ¥®B?_W´ë"F?sFs30?¬Y/è˜2Ñ?¿+ÃI¸¨?ïqo+ë?‹
ÓqfÑ?jfȊ=ž+?q:€5mÀ»?
‡Ù­Ï¿?…iÑb°9É?îK~¿+W$?š‹æe•ª#?fÑV֚»·?gѕÚØ^<?©Úþ ¦Ë~?š*RºÜ?îÖlð]"?÷°mÓ?cň"j‰?QBÕØ:ë?¡\Øs/Á?IýðFQ±?ì!oç?ÀÉå‰(ª'?|h7×É´K?€—!ê=zz?½à³è?À[úÐsÓë?î™é,ÏÄ?¢_ûÐú?wúµÒæ?ˆ×ÆZTж?£bŸ¤œ?žx.#¤«ä?í0<´ÍbÛ?¤?­tT×?rÝú@&Lw?q2* ˜¶x?µP:¶!t ?¤$=Ó?ë»Ú >Ü+?¢—ßH´×?ƒ¹óX9?wøÁ[£??¿½wÀçø^?¡âÖ,$©¶AGN4FGL J2149.1+6104¿ßÑ׫–!@mœBÁE°À9®cÂG7ÍÀ;{Š '§@©ù
G'@W¬Óª7?ávŽöS?Û	tBÈ@ò³Ù¶À@	ٗ
ô¿ÔÍÂ6Ƽ¿æÛz_A®÷¿ëáûbó¿ê(úãe¿ïb>ï)'¿ïŠ‹>‰AGNbcu4C +60.32?î8v(Ì?©üöœe7?‰\ÏR§Ül?"¬töH²|?¦!i§Ñz7?¥b¹Uô¾?ãk~,š?΃aò–éo?¼eíã¦`°?ÀÏZY?Òˆ-ád´?ÅFv鸸:?æÎüþK}Š?²vÓb¿¢?®âö}õÚ?¡»þvҕ?ÍNgÂ?°ë¾¥MÊ?醀E=T}?¦3óÖߜÉ?«‡Þ}›®"?"¦í°]3?ÃK£Âg?¢¡¶=@?ìOÊTç'?¶lö¼IÖ?—ð¾Yòƒ£?œ.ϖî¨ñ?·ŠêJ`?³Ç™¤YЧ?Øõ™9¢c?Ïqü"+?È;ª{F¯?Åzښê?Ú쑈Óù'?ʸ'/×wå?ãC-%ÊaZ?´£é\Ƶ?¶žtÑ|S?¦°¾Õ"?ÓÒš-Ø?´œðä¹Ó?àúål‰t?¼¯°¶…|p?»Vº|¤R?µV
?é?Ùƒ†‡Ä?¿Ij¨Ñ#MIXED4FGL J2149.6+0323¿äÙ:;¡RÀBNpCßÀ9Üëô°@¥À<F։äð°@ú‰*`¦´@êOyº×?¸N\Yr7*?«yQ'æ?ñS(ýOL@$xy8{¿¸tGz'î/¿çOš¿à±Šâ¾w¿áX¾]g¿èöTOãm"¿Ó[Þb¡_âAGNbll3FGL J2149.7+0323PKS B2147+031?ïòC
	?G#it'"?6ڙf:EÐ?&ÅWUÈ<?UÃ?êU­?Crª†.?ïä¶
À'?j£]:U¼?5.w'o/†?D†Ãð§¸?h¤$­°?g¹jÿW+?ï¿¢\¶º<?sÁÐO"Nø?X3ú&ûÙ?e&oµ­fú?z!Óå+å?p&/xf'?ïÍÝu*h?TlÝþ•H.?Fze9QC?''¶Ùm(?v°áúÓe®?S]\­¥3?ïâ#ìÌÐ?\Cw•5 f?M¤Qì	©?@qPT¢?frþkRÜ?W¿Ú‹PO?ï¥ÃAÄØ?ƒßŸŠ¤}?EáýQÞ®V?Vˆ¼±ß| ?…\¯Z*€Î?'Êei©˜?ï—TA9Ÿù?u×F·ð'ã?b±FÍé?d‰o¯U7©?…~­ïŒÌI?qÜ 'L?ït&QÂX?u<íCNœ?]yNˆÁµŽ?I­?#@P¢?GAãKx?säR¾ÖwkAGN4FGL J2149.7+1917?ã͕óØærÀ:ZS2­À9ë—i=±;À<ó"Çz@4K¯«Ô°@·Zï9ß?½À©}è88?·Ù\Á殏?õ°
fóT@%÷5¿ç•žˈ¿ÜX'¿Ä¿çOÁ´?ã¿éxM·‡¿ãĀ˜@Ô¿ïþž
ÇAGNbcu3FGL J2149.6+1915TXS 2147+191?ï÷©~áSå?G=.UÉ H?$0'såœ?²I£"dÒ?LMúFÚ¢ç?DL¿¤»¢?ïí3*ŽÔ?dc'û5°?(Œ½/Šë"?9Ш›gF?aD
4ÑÝ?bg¡ˆQ ó?ï«¢òÄ?rq¥/p?[f©i/Ãa?Xh¦€«C?ªnP²r?p©Æ"Ö‹_?ïæB þ+®?Hv͑ò,?3Á}‰?v	{LÍÔ?gE!c"GQ?G~¹(ÙGè?ïì0§ŠŽ?_O6A+(®?7ùãBM–?5A¥äd<
?`Ð8È-á?["zÿ°8ê?ïÂœk÷?œkºœ÷-?B³´4·"R?Tïz£¹Þ?|¦;3¡ÞÞ?}J›ÀpÏ?ïbÂýbŽ7?'YÌBlñ?ks:ý²hã?m'Í\º1?98übö÷?•0ÁMo?ï¹è"–Û­?f 8˜—?K
sFŠl?8Tš È¸?©Ûæ3±?dëúWŒûAGN4FGL J2150.1-1410¿ïWôÕ÷»ÀFö5"_õÀ:¦‡¾¥ÃÀ<1£Œa¢²@ ×ÅiV?ù»À6âë?Áb@|që€?Â2‹˜z	Ü@€	ö#l@ՑíRÔ?îyˆLj;Þ¿çká©Ó¤¿µWXvb¿»^¾Š¥ò¿ãïî:ތ¿Ôéâéj'AGNbll3FGL J2150.2-1411TXS 2147-144?ïœîîé4ë?™:p`²"µ?Xô|JõÞ?n±«X½Â'?…¥´¯õ{˜?•¾oB×5É?ï™oÎÖ"?j¬~ö¡?]ß='ÖÆ9?`ƒWQ³?…è$´BÑÝ?}æÕ8¸w?ïH¤WžÞŽ?ÂÎ*Ĕ?cûF,/m?Sêþr؀Ý?"lGÕåL?+D¼œwË?ík¢š–'?‰L~p¹Ê"?uZfÆcI?X)ɉV'?³MD¿«.Ë?ˆÖ(–!??ïsu—u–Ê?…ŸŸJ¼?lÙ‰Ä"?f"Èìßç?‹þ£Â9j?'|5-"?ïw"ó(?›ùjXœ ?l"5Àwó
?«X."{Î?ší
O§Aª?–bÞmÍÓ?îVïÖ<7>?•é%ëC|Ï?uýáýÁ½?qf]ÆÉl_?§ÑF~‹g?"sHœÝä?éô9Nïëú?¡Àéö?…ü5÷Üæ?r{2P·3þ?ÆÏWe0u-? ï3MçAGN4FGL J2150.7-1750¿ÖaŽaz½ÀG¼Û¾WïÀ:R}ü…!=À<ZS¸ä¸|@<pšœÎØ@2M	žs?¿Ã±ðþZc?ŸªžÆ÷m,?àv©ò´h@·FRʨ?ïî6>€nO¿ç8å#Û§[¿ç§¿Í
	n¿åà½D™¿äÍcˁs2¿ïÿÛb;ßTAGNbll3FGL J2150.5-1754MRSS 600-040574?ïĀ™S´Ä?pÒ×ßj«?Qm¿,?CfüÙòߍ?y|,¯·p?n–I!Ä?︁l.Úç?{ë ,ú?Rå/-5á?U)ïksó˜?:P"
ï?y¯¸?ïMœ^¬	?€IHc"µ?hå*² A¥?`¬î²'?"/ÎÍùŠª?~ǖCÜW?ï£&²é™.?asµ"Ò·?`!Ì°&·?C9&¤ì ?ƒ
ÞVÖ?^ÇAË7™?ïDSù@7?ŽO6ÙaÙÚ?g'2¬'?]#ìFwL?"ƒ`k+…?Œˆw¿FÖ?ï5'ò?•ÈՉnZ$?aò¨; ?mq@_"É?—Úø¸È?"À^Ûã?îa|ö‡?•"uÏfº?}žØ¼Oí?uC…Ñʤ?¦;+ä°$h?"Y™ÉÓ?îürÜg?}>E\>èô?xi­ÛH?bÏø6™*o?šW9;¤µ›?y|OQ7]AGN4FGL J2150.7-2810¿Å±ƒ Â~{ÀIâ`²È?À;^Ý÷—À<",·/¢@ 6üªàéº@%…EN¾ª?Ñrª?ÄÏi_?*¸?ôKà©"£™@ì&ØÜÐ{¿ïþÁ?|?ïþtå…*w¿ãàH	"
@¿Þ¯°ýcmŽ¿áøžö{¿àÖv~â^/AGNfsrqPMN J2150-2812?ïîûµ1is?[BЧ¨F?5)§ã6ä?3/@A@¨&?\¾+Í¢Ûn?WŽõF™
?ïÐb¼&¦?t½t~zÙä?C…"E\?O+h0*?uƒ.'t@?r& ø»l˜?ï#[œ*e?"Ò¹M?Xb'
ü¹?bÇäâk4?‰ªÖüÓ/$?ƒŒñ'ž1W?ï¦Ç³™†5?g ]û­8É?K$/"gï?3i2ò‡pì?"›ÒøÝ:?gc&#?ïם½·þV?q•ß©áùÏ?I5kcîÝ?F/GëNB?q
s´ø+¶?oD¶Ø_£7?ïzJ+rIŸ?Œä(ŠU?Uøw|¹'?gâNûK÷a?Ž®f9­¼4?ŠZÞóÀ×v?ï-pü?‹ÏÓ)—¯Þ?_ÅBíŠâ?cÊúxšÅ?˜U¨b'?‹L£íf"?îã÷˜[½?†sÃ*¾n?a8óx‹w?T`'™ÉOu? ­[sû?†C¬WU_*AGN4FGL J2150.8+1118?àõS2úJ¬À?»5*"8	À:å!ÁçãÀ<2\sž]@¸ˆd@H{Ã?ÎÁ".öŽ?¦cžœ?Õ=îãx	ý@ý]žk»e?íÜêâ6–j¿êåídòÈà¿ÙziÓe¿ßÀâ³¾Þοä´Ó˜A¿Ñ–éÜ'2ÊAGNbllNVSS J215051+111915?ï'HòY›Ÿ?³½mÁöñ>?4ö"C>?!ü¸±ç?‹
FÔ&"?³¾Ÿ&e3O?ï²GyLƒM?yߖ"øš´?PÙÌ㾘ç?T;oŽ§??RèA/Ö?w-òp9ð?ïzʦNUE?tôÁhٝí?WÎl*éÂ5?=®&µåÆ?ŽSˆólj?tÌ½˜/?ïvB4&?d»¸DUù?ROÅDØa?16Q¤¿=?½+uøË?câϊm´ë?ïš)ا²?yÙrôP‹¿?Ci»SR`i?2øÅ9Š¯)?ˆ>î'et¤?y4€Ûr°?ï7äŸk.'?'JëÞ ah?['¥OØtê?fMæ'Ȫ?—JA˜‹?6ºMڃŽ?îøa67þ?Š•4°
õ'?`;^<½Ë?PZžLdvÐ?žì{¡ôŽ?Š½ž™6?îz)àµH2?"z@™ëR?aþ}Þwü?N®Ü#òR?§=z/"?Ð²µÌaŒAGN4FGL J2151.4+4156¿í•ÏrkéÀ"͒·þ¯À:_úŒ"¸'À<Ib(D€@ [ÿûù5?ù´ýö°Ì?ƙähŸÒ?ÕNŠø.%@«dÅ|vs@ø~©©1<¿é@¸Azsº¿æx6ÝâžÆ¿¸ÆÚVM?¿ÐäK3''¿áñBwô®¿è>ôÈAGNbll3FGL J2151.6+4154NVSS J215122+415632?çÔ]Št¸?ÁÛùNv?¤-\õóco?\¨ÞBç?Ë£2™8i?¿b|ßµÌ?ëj]²¸¤?»+ç¶f?xƒ'¦-ð?Ž«j®Gò?Á—êq<G?º§'îþÈ??êGXT…,?¬ÝàÂ^Ú?µ¯3 ˆ¤"?¤µ§,¯T?¸Îøóˆ?¢Ha4ü  ?íJ¯br¾?ˆ¼Ò'"b«?z²c!u?^Èé²C†(?´ÉÄðåz?‡Æœrl" ?ãþ»&(«?Ã2·úÐÀ?§ÔPD~¼?ŸVO}h®?Õÿªçí?Áàþ€<"?æ{z¯@Ó?ɯQ|I|¡?†üí+0>?"ƒnxèü?ÒQ$\£ˆ?É?eNA	=?çð^xõùÜ?°£Ó!ƒ;?¹'le	î6?§ú1zo‰…?êÏèÇ:x?¦êF.å%?é1'ŒèŽÓ?¡â—sId?ŠÖÄö©:?x%5Ã(,É?ɌI~="?¡Z¯=¹¬±AGN4FGL J2151.7-2749¿æ»à'óÀI-ž×ÆûÒÀ:ªDkiÛfÀ<0®û*®)@Ó/Â"'@[*'ñ¶'?ÖómàÙ??á4±¸tP@$è'4ù@
f´¯Êˆz¿àÃNžÉ"C¿å–Û¿
¡¿è¬R¾éµ;¿ê¢"FY¿ïÿþøþ"?ïòª¬çT8AGNfsrq3FGL J2151.6-2744PMN J2151-2742?ï?sûFÕ?¾R6óK?•6:ë b?¾¦H9ð?fÚ-Pw¿
?`Öà–V?ïƒùqc?¸
¡XO®?j¸Žn{<?uIɤX¢?ˆS€6šf‹?"ÿl;¥c ?îko"Ný?š'<$Õj?"aa¬³ËÌ?"{˜*Bo?ž0»$Qð˜?Wì²°|?ïežÅ¨kD?xéM‹"Ü?Qq¯¾sÁŒ?>42;q͔?'5X&Rg?x÷üª Ø?ïÉT†%Y½?'.®iäbÿ?`QþÄNuš?€4mõ@ÔE?s,½'±?l_–¦½žý?»©˜?ªCœY?{ßo-¸Ê?–XŒ%k3%? é†\t î?¤=¿.LÆ7?íð§xææ? Œ'n3·?—*×yax?•7•XòS}?¥`·{ã?–´^.+?î#P˜…Å?™	v m³¸?`å‹bÓn?VüѝÒ}?¬¼ÅAJö?˜™žîé^AGN4FGL J2151.8-3027¿Èý(":ÀIb@îÙÀ89ÔñhŽÀ;¿?úÁҞ@æ°d@ýÙ<FØ,?¢T=nöWá?Ç°|ʀí%@è_^4h½@{Ã;~†C¿Ó¡ZX;*x¿æ‹a]¿ë¡}¾œ³¿ìàYq‹^¿íS›R×=i¿ïéjÇôö¸AGNfsrq3FGL J2151.8-3025PKS 2149-306?ïwÍæÓ?Ÿ7—=k<Ü?‹Ô%bŽ`C?B—õŸ?i©NÝy"x?n¸qó ÂB?ïÍ~¥™Ïl?xݧ•L¯8?L´;D¶Ä?\µ…_/Mf?u½¶ªÜ˜?vŠg.¡J?í'éïÙ}p?¨w;Öð?¦ƒrµÌ?ŸQ—h™ˆ?¦þE""«'? ÁGÕÎöj?ïñ¦:粁?E2'Œa?Ï?DÂ@\éN8?5¦Ž£€H>?RRjC\b?= ú¥¢t?îçßþøÿ?¢œ·z7ü?œ˜º¤ë­?¡gÖUœ§?y­O×ì?z‰?v?ïn‡wJ?"ф]‡?eãöª®Ï=?|×?Žå:ƒ"Û°?'ÒZS©7?ì2VªdJ¶?°wƓ«K¦?«i(Ô?¡¡°¡ˆ?°ã;ù"Då?©»­h?ïÑ3EÊ?gù'"øä?bv°5'^?Xù}ؼzà?l<C®ÿ¨?`4Òz¢¼»AGN4FGL J2152.0-1205?퐰84ÀF¹‰›õ"lÀ:Îÿ€¾À<k¹›— ›@ #Ýqµ¤è?þ%鞔«?Ñÿm]ü_?Ë!]•Ç?ýíG+7¼/?ÿ"IŽ¿ïýPÒ8r?ïÕ}«&‰Ø¿àÛá¨&$W¿Ûf®_ÏH}¿áP«>¡%¿ïÿä¡Õ¨>AGNbllRBS 1791?ïÈðPNeØ?p[HCYF?HÿX~ªe?;@'¬/ú¯?xgôž^?nÙ|cuì¦?ïšûæsp?"ž*ú‰ÜS?_õû'$Èf?dn÷$†±?…€¡~‹
?€ï#ÄjO—?ï[q½~ór?€¯­SÌ
#?jž[S*?gi
öÓ?'MôƒÙO?~(¿e}× ?î<Q¦!"¡?€²ŸCa‡?' ‰%˜Â?dxö˜™… ?§µ]yÀ¦È?Ÿ`ç¤$?ï"#Ösêˆ?ù®
¹5õ?\'ÕcÌê?Q%óÁœ?‡cX, v@?}Æÿy¹|¨?îÏ5X+'?œœ¥d>s?u:^Ýp]?€Ö'D? jc/¬d?—N:(M"¡?îÊ~8¬~?¡L™Ë=?tŽG;6œ?rRß/ÙÂ? ÆS'ŸK?Ë&ëho?ì4K¯9?—ë1¼»‡«?'ºÇ÷ü?zi>ìÔô?º­K/ÜÅ?—k1¶¸6³AGN4FGL J2152.5+1737¿ÀçHŠ®À;°¸{Üð0À;óiï‡ãÀ<aŒ¤¾Ê@zo÷ß @å^¼Mùˆ?͇4|´['?¢tâCñ5Q?ҝO0¿»l@ŠšrÝm.?é'Nž·Ì¿âZi7Ñþe¿æ]¾Anµ?¿ä$à¿ÈØL¿ãÎAvÂÔü¿îô›GðAGNbll3FGL J2152.4+1735S3 2150+17?ïÎ]LŸY?g€"âÓ?9øÍö‹Î?'ùHê?w1Ípg?f±'j~)K?ï§8ó³ã¿?~U2×®«6?X¯…¾lI?bÈôz?ƒÒQšŸ"?xÒ¬0P?ïf€}œk?|o˜ÄPŠ.?a7/1g÷K?W8êþ¡;;?'	
b&H?z²‰fK?ï? ÇéÁ®?psG­¹F?Y¿€¬GM?:6q®|€]?–oõ3ÝÍÝ?pYRõwé)?ïr.՚?¡?'|òºŠ9†?M÷k–#((?@'ö,*¢?Êiê+6Í?óÂû×Ã?ï
?#?—fàb@?cfjè‹*$?sÒ‰L»_?œÁ'ZZê\?"š÷¤r?î™Ù
*"?Ž"öùobÑ?p%üsðpù?h)Ðmrž?¡Ñ¢ãXû%?ŒW»‰K`?í²N¼{›Ø?Ž
Ӑ
é?nÔ{åÐ+?Y҅€(u'?±væ;Ë"?ŽPÐÆå(ÐAGN4FGL J2153.1-0041?ìA5ÒÂ'ÀC߸ä¸{ÝÀ:é€æDmÀ<oèPïÝ@!æfRDpr?üÿüB?Äݦ¨ É?xCGŸÉ*ù?¶»]û)@txÍÇ?ïêLÚ¤%å¿ë^°ô)2¿œ›œNª³¿×«X¾ˆ…¿ÛoŽ˜´—L¿²WxÅ8¯AGNbll3FGL J2152.9-0045RBS 1792?劉œå?†€œ¿á#h?2×r'Æ?%–¦Ø²O·?…‡~3îŒ>?†`û¢¶q?ï¿ÙÓVºÞ?yÍFÂv¥€?H¥=Æ+Å?T(ÉóŠ˜ù?|þn¢ûc'?wHA%ÑÙ!?î´|\O"Æ?–œú©üT?W"Z·{íº?`ĐƿË?£û—gDšª?–©/ð?ï[ï,.m?tå¥?DBuÙ)ü"?-xá3–³¹?"ûŽi*_&?sãÍ´Ç$?ïd-ELT0?‰ã̐m¯?A¥
TC?4¸ó¼NÊ?'í.'y‹j?‰"ŽZ°­?ïi؁h?Œ
å¤h?QC5²[Ü?]&k4…;?'°¼~~"·?Š—Ýâߌ?풺2I? =Æ·™eÀ?Y+ì­ëÉ?V	Ä0e][?³é½J-3? H¤FK?îTö_R?'"Ƨ-|?ZSô!¼¢?M'Ú$=®D?¯ü~Jœ?'眆Þ×AGN4FGL J2153.8-1137?ì…?RåÀFÏËÉdcÀ9JÃÿž±1À<çq"Á@Øi¼\<A@7bR¯'?­'n®ßQ	?° ½ ñ
?ü'*߈'@›†é_¿Éó£»±q}¿åcn.±Ä3¿çBE¿é}þ."¿æà+²~m¿çÓ`žü/AGNfsrq3FGL J2154.0-1137PMN J2153-1136?ïöT@Q²X?M+ÞÀz͙?!3ñXꍥ?JŸ•IÄ?Q1³™	?K[2	vN!?ïäUp†.?kʇ^ÁÉê?5*^ƒk²û?C­f
ó?iCjq»•?h‡@¦æ?¯?ï¼Í.ã ?i%KTl\Ø?UFw!6hí?T…N»$Zà?|GÔ½ž?eææJ—"Þ?ïáþÏ?JÂGý;O¢?L£ùñ²4ý?21¬ŠÅ?g¹_ËË{?FpëBA@?ïåÔzb"?cvOÔßÙÚ?2"Hß¾?)…
sR9?gÙ$€\@§?b~hçþ2?更>®ç_?ˆwOôˆHQ?MùŒ`À?_½µF5&?…" â+?†»E4bE?òuË+?yZE.Ôòë?`iJv·?WÃ°?ˆýpÄéG?wN¿çp@ø?ï®Âyü_%?l{‡à´‹?e"µ_'k¾?Tõ4£_eø?~
hA‰—?fò_ž@0hAGN4FGL J2155.3+6602?ì>\Ò=úâ@"	¶o"5ÒÀ:êg¹MÀ;²ÎºÖ¨@Iß,ö®@p'ݽ¶?ÉÅ?º«3?ÈóÜ܉0@γ!*3@Ý:ÆF¡?Ë*é£OA¿ã7ÊaŽž¿êdkð"ò¿å¬"½ð¿î÷à†=¿ïÚÀ«VZ€AGNbcuNVSS J215520+660839?ê·Žn¢?ºb¤­ý\j?'¾]Yˆ˜§??ɏB¸?ŅV'!?¹~<Þz½?ê…cµ9¼?¿pnۈ…? Gζ0þû?¢l(sñÒ?ßöıº?º¦5'æ?뛦3OŸ?¥Ï5y1åÃ?œ\?{Rø?§,:	€?¼»Ÿþ¸'?¢l"æœû¦?ëíâí?ݙ>N? ãnPŸè"?{(B¢e'Ð?¸%‰¿kl3?‹Ö*Þ>Ô?㊡Ñ÷Y?ÃsU*\}?¦Ï?3j½B?¯ö`X—a?ÖÔuÚïó?Â#yÌõ''?㴹ۃsè?ÌDBúü`?²ÏÁ&R/?·#šìƒ`?ÓâÇw#?ɇ'[˓ù?å6öºîL?²‹ÎZ	™ƒ?´©B‡xª˜?£M¬˜:N$?ÐgÁè¿?¯5(´ŸÇ?åL¬õ?¤Ù½|I?·:µ×"†?—©ˆñ¢?ÏEÿòÄ_?¡Ë"Öp–AGN4FGL J2156.0+1818?ìR%|'KÀ;Èf^ê–À9æ7UãUÀ<-5Ã0l@!ŽsöœÕ?úP¿54•3?º‹ÉwWÐL?¸š¾²­¼¼@:g9Êüé@ù0´¨¾¦¿ê?ßÿY'í¿ÂI#ŸíE¾¿×yTŸêk™¿ÑBõ"ûƒ¿Þnê.£ˆ¿ÒÕ½aIñçAGNbll3FGL J2156.0+1818RX J2156.0+1818?ïÞ"¢8Æè?awE<èA1?<ó,p1Ë?0(•B
?n>üäÈd.?`a¨sŸ‡Œ?ï¿Aáþ&?{Éc»ÛÀ?N™»>GÞ?S½RJ–w^?|Œ> ÓÞZ?x²¸@œ?ï_ÉÚôò?}€÷²a»)?e-ÍÔ?`jc¯>?'a!niÞú?{`Xâo£]?îtòê r?z1lÛÈ;?qyxÔâw?R¤ï5_ã?¦p"a	?xíeµš¸Ê?ï±p ,"ü?tï…®1?U4	"¢½›?JYÓõ?€ýv³D¡T?rÚþ¾tU?ï<AΛGÞ?'etú¿?a³E]ö^û?hªm¿²›;?–A]‡3M?!çÅòI?în±ÛÒ·?•¢¡m2n?z¥éâpó¿?{4%²¦±?¥À%	#ë?"§Ù‡Í·?ì`ÝÒrlô?"ówh´x?'
LSøÔ?oxÝè 5æ?º·ÇíiûF?"—Ú\AGN4FGL J2156.0-6942?ãN¸Z'‹ÀDH—žÖÜÀ:T}á­.¢À<((@éÈ@rK'ÎÉý@Eþw?ƺøcÿXæ?Ôûñ}†=œ@3öÂiœ|?úpH»ÊF?À *Aò闿ÌĈZ¬ôÀ¿êôZ5Ö|¿ïýA©î{s?®-ýê&$¿ïûpÿqºAGNrdgPKS 2153-69?ïM9½¢³?'­R÷\O?o¿NO'f)?p0&àÕÈh?'`ހîâ?Z§†æ:f?¶¼Xû?¦Äþ¹cKo?ˆÅæöæô
?•þ¥ĵ®?+Õ°q"?Ÿ{Òìóõ
?êï*	¾Å£?©zg‹eµx?§uµŠ?š•80Ôü?¼öï0á£?¤/"vZKç?î€3,/çW?‹ßEº
FS?ƒÝϯýH?w'ݲï?£6•È'š@?†|1
oþ`?î1zZ}éª?©‰9K¼q)?‰ÄÏÒ^•?‡ñ"™Â™?¦w&ÙÅ?¦ÜÅÅõ×®?ëãþ¿?½JãNՌJ?¦FÇõÏâ?²î4½äâ?µ¾ƒ˜ÅA?²¨iå"¹P?è¥a\w‹c?¬2ôö–ݘ?³˜=©!ژ?¡üg\7l?Þ[¹þا?§ÿK÷Ÿê?ëcÈÇ?ª(9's0{?¢¨ùFÈÿG?šðúÛQ?¦?¾€ey©?¥-°þ•AGN4FGL J2156.3-0036?ךQ›ºAkÀD+¿@OÂÀ9é Ï¨À<3ëGWL@+ót¡@ÜewS?µæD1?œöCW‡j?åB]"<@µýM?+¿è è½ïk¿Ø.}`ä¿æ'S‹'¿á' ¹Ée¿á~ˆÑË9O¿ê–ÿ5¿AGNfsrqPKS B2153-008?ïø[܎{?;ÿ-&†‰?"¬.÷!s?¢•"¼¢K?K=å­v-?8ÖÖL³É$?ïë­î:ZÅ?gr²³?&²µ‡Ì‹Ù?5Z«Yöµ?bææ?@Ýî?eäBå£Ík?ïÀ¹4½f?g]d=?Ro5à3u?@ìgÜî?{¢ä®"O?f{
梆´?ïîñ	Hº?@€úa$œ?#fp\N?	3[?_»R×^eW??Ãý‹Õp?ïñKÚsÿV?S­7¡ýú?0×Í@ø»î?"#«iØùÍ?Y2WªY¯ó?Qe
Ã.ŠÏ?ï»Dâ‰?€oßkŸÞ?7æN‰õÇS?HÝ3ŽÛÏ?€zü^)'á?šô/`Ä}?ï—lRL?uŸÒ¹FÅ?]@ÉΛv?\GÕ‹?†|âÌ	û¤?sV¾S¾h8?ïÔÓ
ËØS?^Y
ÜcM?91}WÄå?'!8òmœ?t·—3øP?];N¦AGN4FGL J2156.9-0854¿Ôµzö–JÀF]xÀ:"¶ÂŸLaÀ<z™_·ö@œ¾¨Fۇ?üâqy¿ß?ÌÙäwä=,?ÌMbI†@ê̒@p"³¬¿ÜM[=…¿åÅý_çœ1¿Þd}§ö¿Ù)*›´üÌ¿àRh' Xпïù–m•/AGNbll3FGL J2156.9-0855NVSS J215650-085535?ïÁ(qcDž?lﴟ٠'?K뮜Y?@!òc.ê?{ùãª`›‰?jΈtêHð?ïx<
·?'Æ[h¹Vh?[Ûƒêã?[6$ZÏmµ?ˆ¦Ž·¢Êï?€Ü*œ6†?ïj°û¾A?{vŸo¢ŸZ?l=6¾Þ?mDpn'Põ?ŽD¬ñh-?u³ê$	î@?î®]@Ög‰?wé­B?Øð?o
ÝžÁ‡?R"É¢+©ž?£)~"¡"Ú?v°5mBI6?}X+¡?{#/Ào?^ï6!+Ì?PN°€îò¿?‹ÿyêŸ!?yN@
¢<?îÙ¹pé;?—¦÷ ìçM?k·´ŠRS0?m0;*O>?? ¨í¤§¢m?•úf8JO?îóߦ¡Èp?‰¤é«ú7?v`§sPÐ?q~®³\?›ëáj1¯Í?†HP‡¾m?ìܽAƒFá?'ö?Y‡?|T5"‹É?iCš¼]ٚ?·Tқ©ûM?'~üÊ(AGN4FGL J2157.5+3127¿ïñò"œÀ2="ôÆæÚÀ8I"ðÅÐYÀ;¬šÚâ9F@_t;@_‹Íþü?¡aÿÏX˜?Á|®¼Áfè@ c7ë(Øf@xhZ†­¿«Íÿý¦´_¿à‰¶b'<…¿ã'7oØÕð¿åU¥ïqó¿ìž–XœyH¿êÒxþn…oAGNfsrq3FGL J2157.5+3126B2 2155+31?ï&(¹*??®baŠcº?'4…'v(?'
KK\?' ¹öë¶?¦U±©¯*?ïÛ­˜Ý›?wT"úw½?C?mÆ#?X))ŠŒH?o'‹Ù½"?sßXõÍg ?íLóbN?¥)/±y?ª÷Íì|t? Áȧm$˜? 9¨^«?˜Ø&B¿Ù?ïêžø[Ïg?Pɚ[=í?<^Í;Xq?/†æ2'[@?aÕFÍ՚?L"u‹Ê%¯?î­Pš{l?§¾J'º ?Ž»ÍBMÂ?ŒÒ'ó†?šøŠW¦?£ p€2?ï°òP6p¢?ˆ›0K&Ž?b(Ä!?€0'°£v¿?~ruÃDŽª?'%HI$ù?ìÕlüW©à?§äÒ¬N–Ö?«á¹vŒVï? …£9øÁ•?¦ÇvÅ°Ù?ŸÔF}b¸N?ïÅ
ÕµÃ`?m	´ÄPÄ?Qü¿À2'J?EÐO ïÈ?xûeQ>'1?jsßïiëAGN4FGL J2158.1-1501¿ïRT7Ý|ÀH<ÈóÀ9G+ý´Ì%À<"?ø="ß@'€ vÃ@¼w¯d?­@
‡‹ã?±"\éü@]Á@ŸS²¯•.¿ã™*GÒ'¿Ú²Í\¿ž'¿ãž¯çÜô¿äRÀí ¿âi%'×µ^¿å-c ŽUnAGNfsrq3FGL J2158.0-1501PKS 2155-152?ïëƒh¢"L?[¬£Tž?-ϔôôÑ?)óGÙw?bŸž–é(?Xµ=I)Ò?ïÑ@2}ß?x1L,ޘ?Ež4'*Ê?QàB5‡³×?t¬)ÊÄÖÔ?uÂumÛÉÂ?ï­) I¤?ycœxl[?V.åò.y?Gu{&?ï÷ɝG?xž{¬üÔN?鶴AÛÜN?c/€O^u¡?[DX(&Û??'£W"ÿ?'l$ƒÔs¨?aL·1Œ?ïȐvŸ†?suZÄÍr
?AO¦{ÑÚ}?4ñh™æ«N?yÏëËúš?r¢7%ÇÁö?ïrù?"3O¢O»?S'ëˆÜSo?bøüXf*¥?†q&fyº?"ÕD¨l?ïWm€¿-?‰ÖˆÆ	O?cˆRݐ?b¸‹Go?'¡E¤=Ñ6?ˆÛÍ+þqÇ?ï"P6ú*?ƒ.(;YC?qRD¿&?^Cã
Ï8?—atL³ò?
ìR&µAGN4FGL J2158.8-3013?Ûõ26ˆþÀJ&k¤"ÉÀ6A7Cc,À:p¢¨6@Y'¹'m?üDÄö>¶?‡Ñ)ëЍ?¤ùÖp9£æ@tBÇû­@ñé…Àè¿¿âÈ6ºý¿Ö—¿¤Æ¿Ü´žØ»g¿ÙÝF'vú¿à;`ÿX±¿ÛՀºûiAGNbll3FGL J2158.8-3013PKS 2155-304?ï•£7I?®ßYŸâ?6¿aëÍõ?9Ö3ù½?Ÿ—­)p?–É#™?ï˝îúz?€W°á¡Õ"?J¾8gþ?c©«-y?víÐÂ>˜0?}2?ÉÀ½?ꗵV
¨µ?²N(w°u?2KZ0
?'‰âsPzY?îñJt\?°·™ag-?ﻟ˜-«+?pÍÝoG?-(ñ‡ë&?Ä¢	?€£v'Q»"?p«€Véz?í©«)[ey?°?x¬]B?IÞdËÑò?G ¢ê³?²~éëƬ?°u¡Yxä?ã¸Õ'?•kÂèN\?P™ºU˜º)?a2UúÊÂJ?ˆüÏÍFë?"óZº'‹Ô?ìWÃ$FJ?«Ôeo÷Z?ˆúçüÏ?‰Ô3`¥K?½T/ÆÛàÖ?«'¯>¾Ï?ïš()Çt?€ìâÉ
҈?2ž£¥—³8?,ϓç¤Dá?ˆá£xq?€Ú¼P]"‹AGN4FGL J2159.1-2840?Ç͍MA8ÀJ<³åuÀ:ŽF@RÀ<AôÚ2@ C¼¹Ú+Û?û<\ŒÈп?ÁDœg)Z?ÄX¾Š@BíJ.!@vðéa­ð¿ïÿülò?ïÿÓ?,» ¿ßep½Wcê¿Ôo……t¿ã#-A+ÄT¿äK"=,®AGNbll3FGL J2159.2-2841LEDA 3218689?ïÎ]|_?}ÒR Ÿäã?I|ŽÚm†?>á2ë݌?u°D£?}Z¨]MÙ=?ï˖!êr?y°\» µ?Ný˜›K=Ü?W
¾
LÂ?vU=D¿,½?u™ù‡á o?ïf¦Ò‰œ™?†Îã…ÿf†?h¤<s{Þ?r‰"G?ž^Šu?…ke	â/?î÷ê&œCd?sÚÓO¶Ÿ?sêHXíU¦?SH5•by.?œ)?r+DœP#ø?ï¿#p¿Ó?w_˜›\²G?bH%B5­Ø?Z—_}u?wJ4í͗[?tÖÅåÉØ?ï]½#Ñ/L?'SÌBÔ´ú?`Š." Ž­?mÛðÃc?'7¬>Ö¸?+[£iÒ?îì
Jݐ?'9Ç·?r´@3ؼÉ?q½é??Ñ¦µ½º×?ër'4C«?í×`=4
?‹Dx™N?'2Yí/7?lÞИ¦Úì?­ýX£ã¨?‰'ëzŽ›ÍAGN4FGL J2159.8-4751¿êö÷€—:ÀImÙ]ÔÇmÀ:zê÷Z?À<ƒdIU´g@t"aS×î@(?NÊhn?¼í™I'›?" ë!<¢?ÅËÀæå@¿Q$_Û³?ãÁ­Ÿ`¿ãà%¿­)™¿æ9Áø]tO¿é+f ïÀ¿ïýŠoZ*ï?ïßM œÃAGNbcuPMN J2200-4751?ï÷Kg¡=Â?Bh$:.M ?.e‰[{üq?#?&5¡?K8ÿk¡Ú??ÀMcJå¬?ïä•4žÜé?r'[W?5x¥,·-?DPDïådˆ?h»¶µkTµ?pÕ¼-ý'?ï»!ÐEŽf?tO¥kdò?WÏVTI}'?aõ(uéàà?|{B]t¶?rBh#?ï÷rÛ>Õ~?4^5¿q"?ôWºœM?~L ^[í?N¶=‡¹ì?3MWÅÍ|?ïì·B'm?Y0+ž?@²"‰"¨£?8˜õÙ°:é?^8ƒƒxà?W
Rèžÿ#?ﴅ£öóE?†oäz¤?B«	pÛSè?_Òì|b¢?³æwDçZ?"lŠ4ÔJ~?ï…l‹™{½?}Q³Œ?bòuÇ»¥?glËsÉì?‰è?™ó܆?z)xÌ«3?ïãÊ1^i9?WrÁSHÇ?7Ol•pàv?,9O,e?iKà̆h?UȒӜ<¿AGN4FGL J2200.1+2138¿î±BU˜–mÀ:>$þ½
À:-m÷T`À<KvY"±@.WÁ²èJ?ÿ¡mµ?¼×Õ˜8F?°R,—Õõ?ô'p*4†ð@)ˆh™Çg?¾†ýOüm¿Ý-£ùnì¿åœº¶IӉ¿Óú D¯¿áƒsR3Ñ¿ëwÁ½¥AGNbll3FGL J2200.2+2139TXS 2157+213?ï÷ŠŸš~`?9üé3j?"K­£ŸÖl?€B]º±	?MB–;a>?7k1 קê?ïé`¥B€i?jUòs?0÷t-;??M	"]óÔ?d€l;›
?g—è"þ¦?ïÄl™0h(?j­>€.·?S3ó­ÐH?`
Ø1?xü¶™4'þ?dyoiܝé?ïÇ:œ^?SÈFÒç?B)Ÿéõ?#_¬F`?z}Â/È?S9wrÐC?ïñ{ݓeð?G­ræeö?1{…ÎË? @Dq›?X©~f©×{?E38åÕ²?ï¶wXڕ@?ƒÔgÂ"L ?D…ÉBã?UIÌѤ'à?ؤâo?''»ß(iã?ï  e"ô?pË,»¬2]?[§ÏoBô?V6«y<?"—q¦TuË?lÆC—î—w?ïg]0K'?r…Qì7rq?X‡Õ.¡€?Bš¤cå"Û?'‹Üª€ë¥?qí2t¦­ðAGN4FGL J2200.3+1029?ï—Çñ,
áÀA.@…+NÀ:x3|.NÈÀ<PX(¶¯@¶Z
'º@ISù|X@?Áñ"ÂÅ7?ž¾}‡Gåû?Ú¨Ë%WÓQ@I$ß]s#?ïÿûB«÷¿äÜ)áû³¿ê²îO'¿×ôè_Op׿éL÷?7á¿ïÿ¬)ÜrAGNbll3FGL J2159.8+1025TXS 2157+102?ïW3òº‹ñ?'9Ý:eþù?d\õºZ?`´ŒÇs¦|?'—€;ƒ÷Œ?WëçS½–?ï«ÚJ¨‰?|dö
ˆ¶?WNÂh—Y~?[ßp¡þ@?'•@î§?x%ÐH&:I?îIö0seR?šßÓoI?x"ýÄU Â?z,'ð­Î?¨NC'—½?š"ÏԆX?ïnКÀ>?mE4*±A?sâD]Šo?WwC6@?ŠŠCÃ×¹C?gÒ:f''Ò?î°×‡Õ¯? ‹ö~†?yȼEåÃ6?t>•¡ÆC†?¡¹où'F¢?Ÿ:–ZÉ?îï P0Þ´?šOz€h‰ñ?mŽ9l\›?w¸.‰C×?žZ5MB÷?—1b3âì°?íɋ±›æG?œ¢'ín?…ÔB
hŠ?ƒˆ&gæHÀ?­ò4i­Ýb?›¤Ã9TÈ?îpo
Ç%»?‰"Í.£U?Ü·šnRY?yüRFTëB?¡ák:A¸?ƒú˒*žAGN4FGL J2200.7-2414¿äÅP4SwTÀIÎWâ?$ÙÀ:•'Àa"À<'F…@J'KÇ~¯@e9Z"¡?Áþ{
ã3?©¤2|]?æá¤_Æ95@
Ô‡Spë¿çtî>Œ'°¿Öµt@™£*¿æu9½æÕâ¿Ùè<œh¿æ'Z«GA¿ä)~HÛ;%AGNbcu3FGL J2200.9-2412NVSS J220036-241428?ïñy§-Mc?lXµÊ\B? 9‰½œ@Ý?l'­@N?[€s1Û?k÷Â#èpÏ?ï妗Öi?j"!ÁŽÌ?2m í'Âc?>¯èEIØ?h´æ:Ø?hHñ3Õ½?ïÈãý«?c7ŸIøï°?N8Ä̽Û
?4z-ÞaÏ?wÆè÷˜¯ç?bpA&«o?ïã1ºÉP?GyªíÜö?4Ö¹¦³,?mk¦0?iÈ
J"ºG?F³'YÊb?ïò€¿ÇÅk?Qv–$9.?*~-ø¬U?d9þ´?W®¿‰­ê:?P—n…K[?ï­½Kqæ?†Îsk´?Bì"…û?Q¯Ôú±Í?ƒžÁêÐ&Ì?…^fF?ïªã£vµ?q´…2x[?U6Ý°Ìpn?Eºs녰?' ;Žg\"?p·|@àËR?ï²wého?fÔٙ"?Jø@ýÇë?6©ZÄ¥º?²Ÿbµ?eÐÓO€®AGN4FGL J2201.0-5907?îâD'oÀGW}|,¡IÀ;:p>V}À<ñ8Ë@ ¥xJŸ?ýs¸ÿnx?Ô—ç—S?Üþ#[ú§¦@gGzÕ@:ԈØ׿ëU ÃÄæN?í®ðBóš—?}Ö¨¿âGò½¢7x¿éØb,E¿ºRÅʤÿAGNbcuSUMSS J220107-590639?ïȘq?nX/!ÚD?bm‰?\ÉÛ<¼rÜ?r¾}&bê'?e &
µ¡q?ïJÝi'5ú?¦ÛJŸþÿ?m(\ñ—ºK?u˜ÂÿÐw€?'ÿG7:î'?¥¢6a–?îeðmÌóI?•»iʊW{?ŒcÇS$åõ?‡ÔÙáˆE´?¢ˆQ×-ç?'(;µ6?îÿÿ!¼Eõ?}œ×xŒ­?~<znV?oôfî?˜pý+)óp?xAëONß?ïlgtƒ_›?é´®¼w?€›¨{Øh4?v0Šoƒ¾5?"Jzq¾Û?t¥pXRàv?îN3ùD?®£¬3xs?"Èl~?™Í5ÓK—?¦+nÌD?§
£3UªÈ?탉î?Ÿ~'ÙÁ9â?"šû§'b?Iïj§?­ùñÉ—ï?šŽÌ°¹?íá'úá)?–:/½.o?…äµ"–j×?'	+ ä×Ô?¬m³
#²q?"Z#á&c&AGN4FGL J2201.5-8339?ïäÝüÀ?¶,ºs-õÀ8¨á¼©iÀ;j¥P‡@ž«"‡@î.|M•?¨ß T« ?Âü]CÆS@ï»@ãÑ C—Y?ïGòrxÃ`¿å&H.ÿæ]8TÛ#¨¿ç÷#b…±/¿ëãIEÄ/o¿ïþâ=ø3-AGNfsrq3FGL J2202.4-8339PKS 2155-83?ï×kŸ
qÉ?h1;›¾`C?c
àzÒ ?\ÜC~*5‡?eŠNRì\š?_yiD‡"q?ï×<ˆÂÿ?u|I]'
?M#!Èä¦?l"Q\h´"?p½™éI©ó?n‰Ÿ1þ:?îƒbú÷?žãž
ò–C?™€‡RXã'?˜4Ö'gá?–lU'tš?'îÜh·~¦?ï§iȽëÖ?f'îé±ü¾?`Kí¾…Ép?IÙP.le?''^#è6?cOb‹áÛ2?ï´mC`Ž?t°øL)¾³?o'X,9ã\?l{åãÒ?v²)Í̯?i1Û8?ï‹&µTÚ?¬árÝS?a'±àú?uÔÇêÓ.¤?ˆìfw³?ˆé"\,¡€?îgèF¥×?¡Ðý¿ôU? ()>èž?š³–üÎu®?›´²¤­sì?–'~,Ó3?îóödÿ;½?…<^èß 8?{ϳb"³ú?ivMV?šF4K^?ƒŽçjÜžAGN4FGL J2201.5+2950¿ìۀ¸]eGÀ4ë9Ÿ]ÿÀ;×gZ'À<ˆ~aßï@@)iÛ»Ó@^ø³Û?Ï7‰I`œ?¶¼¬™%«`?ç¬ÄÉ$¢@k—ˆrTÜ?ӇŒü¨1¸?ïë뫵%¿æ⤥fVv¿×–£EG¿êaQžÙ•?¤,٧ѕ´AGNbcuRX J2201.3+2949?ï£üpBL?'ad"ï+Ã?Sââø?Td-.ø'?"ŽÑÙ?æ?€v=Yá͂?ﳁzû)?ø¦I÷4?RÞx^Ÿe?Y0Bb8?€ÃÒ*ÄI¨?}k…úËKº?ï[1|æí?à¿~ »í?j‡Š&úµ§?p,üwO?'HÝ߯?ᜱ1Öß?ï*ØÜ®ê?sA{°Ý{n?r4øîw[?T0M»JÊy?–¦3ÇØ?qhž»¹?ïC'\ä]?ŠG:`ªãå?a¤±ø?S»(Ç×»?•xÙ8H¤g?ˆøâ³ÑÅ?ïJ'Êö?'"Þ? ³?dõ	´a)'?rhËv§a?"k6Ë<?,•dt¬w?îÞâ¨EÙ?ŽR&/Âúâ?qRÃl‰ê?rż`æ™?ŸÎú&Õ6?Œ]hOš~
?íÇðÈ2;ð?Ž/ "{Õ?ƒ·ÕÚWÇ?p_'6Ý'?®",Iãb‹?Œ\êšEĎAGN4FGL J2201.8+5048¿îᢃ'ß*Àdg`ai§À7²š²žM^À;L(Ê#¥!@¶Ý®òFY@€_†xT¥?›öAô?Â4J@Qü£T-@ ·áXJ¿Ôy!Ôæø¿ãyk@Àºp¿èÊ÷uR¿éñ‹@;¿ì¥2Ÿ9–¥¿ïÿ»!(ĚAGNfsrq3FGL J2201.7+5047NRAO 676?ï[H®£±?A1êØ?~¨jù»EÐ?~]›+2?‰ÙžÎTà?†"ý1ÎÂ?îˆÝtÃT?¸B£'jm?UöiºÁúç?p
7?¦ÂugØxÊ?·'ú"ù¡?î¯4¹£­Í?œ'à"èò?—‹¯€?•ñ¿›B?'˜U:³Éà?'?Çã{\?ïðƟ"¸è?I2"U€xˆ?7§rȐ?,}?«^?XˆàÐý?E'L©â?ïJ?ƒš÷	?ŽlKŠÉ?~iqÇ­?}ݓ§èÀâ?Ž;"o|ÿI?†³'|t.v?í³'£''?Á"œÀѨ?pï¹ÅãÁ\?˜t"R?¶;g×w0?À큷Çú?î4ÉùŸ
?¡Eëz!J?Ÿ‡óç´RÚ?™zc¥?™ÞéÕ¨/ã?"¥Y§ç?ïÓ3I62u?húýX!&†?Qûc›??IM=Â-Ý?q炉sbù?f>üâËAGN4FGL J2201.9-1706?êð§5A3ÀHØ#|ÜÊqÀ;Í¥,tÓÀ<Òï ´«n@$/ÿ¨Â+‰?ö…6+‡?à«úYÍÑ°?–´3<²&È?¬ÊÎþÙº?þ¶ìM›"F?çøäb•¡g?ÝYŽÏ[¿å>^‡tÔ¿ïÿZS2¬û?ïþSW•é¿Îîì\_&AGNbllRBS 1813?í•![´œ?¼•×¾ÔwÍ?:ƒí=ŸË,?GŸ¾QÐ?³<q3>³Ô?¼‡ûŽ#?ï'
2w»<?"E´GÎS?b	^®Ð"C?tÅÕ¿ìò?†û½ìLS?¢däôu?ê0_0¶#?±Ò-—!v?y"ٓÍ|?'òvYj€Û?ÆulÞЅi?±šA"Þì?ïD~s?"+:2^"?" ÜT ðÿ?)ªÓ·Ò\?Ÿ9Õ¯a'q?"*¸¾·† ?îãöK^?¦¿&#³Áì?F)e½ý>P?RƒptöŽË?¡gù訏E?¦ŒB \®?ï&e¢k?¤o¶í΋O?iíÙ:°n?†u}tcÃä?—õ¢h|—?¡­YùrQ"?ì"Óöš?¥³Y8?õÂæJF}?‡œ/µ ~?¹"®Ê'á?¥†a4v ?ëîÂJ½¾g?¸€ˆŠ—aö?1ÒÌ2«P<?@º-¡J[?À<
nÊÛR?¸€åá6_dAGN4FGL J2202.7+4216¿³r°Çi©À$ãb¥ç…¶À61â§)¥À:¤Nér@¸¨§ÿc@%@FA,ñ?"•1f:­·?®Õ¬€?T@$YH¾H¦@ UšSÓ¼«¿Ä¿('!-¿ÞýÀà…f\¿ãӉX=¿âÐíޕL-¿æ;a3v¥¿å(ê¥$èAGNBLL3FGL J2202.7+4217BL Lac?ï0³h;—u?˜¾Y}°ì?`Æoå²ù?am»'^š?—ÐÒ	ˆ?—J!â'ýË?ïG±þG÷™?©@Œ*Mäî?m!x¤Cj?"îËé穌?"e''¥Îk?¦—«X¸ò³?îRbÔ>8Ó?¢4 ü¡g?'òÜch95?‹X´Þ)Ó?¦ ˜²? …¯Þ¥H?ïÅ¢J†û¡?hb÷3?P|§01&c?EžÔ«Ã'?y±"±?eLý%±r°?íÒì8ÍÑÚ?¥À©qá–I?rÂ	øŸ?tNäß|?°<|—õ"?¤¼©N`_?îÌÐÃã€?¶'Уõ?z֖;ùzà?•Ñ¥Xýb»?ŸÈ@Z"õ;?µj‰‹¯v?î:o2ùã—?¡*Èa \k?'¤1rõ³#?‰hôZû?§°u\'½? ›áVù_?ïw"Ó'Ɍ?"{¹ß]<?bJƒ•*?Zøš"d*?ž¸£†=­?ƒRvçµSAGN4FGL J2202.7-5637¿î'ÃH¶õlÀHÓþuóÀ;WçS`Ð$À<ג:)Çz@ —½çו(?üì*EMçê?˯ >#|?²t\É.²›?è|îh(?ûÊòìq-?Ú¡Ü>ñ§?îÌ Ÿ²¸O¿âsÞ-è¿Ï¤Váä-¿ïÿò~#¿?ïÿ·ÀÌ
ŠAGNbllMS 2159.5-5649?ïÑÿƒCq?qåC¯`äõ?SD°¨»¶?h+RÚé~?r>-N£W?h[3Ϊū?ï‰Q º'â?ˆ7fÙ#?d—¦¿R?geӽۃü?ˆ…Ö3ÌâÒ?"iþêϺ?îÂi~k7S?"ÏÍX
ñ?ƒW…ÌQ?…Ður?ž
ª&sv?©9jqó>?îäW¿žTÙ?"=àûHÜK?}ѶZ¶U?gDæJé?œšu/ٗ?'céS°?ï¼õ"ù¡Ž?x×ò!Êoð?d8ÊvÜ*c?oäºy?wi	N [‡?qôjOÕ?îÝqQ?Òm?›ß××q?r—›oŒ?}3ѱ=›0?ŸËïñÙ»b?˜­øbi?îa`Èö1(?—‹_Nr"?ƒ#1b—‡˜?†}d(¼F?¥!'BŽ—?"ß m{?í¦äÓ E?•=us¢ú?Cû"}÷?ƒh#'Ǽn?³!Ê"*Ø?›@F'u"ŸAGN4FGL J2203.4+1725?l‡	AÀ=£µ¿j
»À8:²ái<À;§I׺f™@•äô¶Ë¯@ÚŸb0w?œý( Ëß?³"a†q@ö_½Õ¹@ebÉ"ô!¿¾¡O›s¹`¿ß:ÆF¡¿åK~îóhB¿å7_ÞO¿æ¡!þ'|r¿érR,ó~AGNfsrq3FGL J2203.4+1725PKS 2201+171?ïòÁñ"?Iވ»ÔRG?1"PMìü?$xn~s[?W—h‡•ðt?Gqu)UÄ?ï陨¡ä?eA¯2Â#î?5pOIj?M+ ´ïJ ?c¸MlÏöö?bçðåóÈ?ï¾¾Üõ?uTbc:¢"?Z
HQ-ð?cµŒD>™Ô?zn]‰E«?q¯Ëc|
?ïûÛ"+
?&-Ö%8˜?ˆ´)é½>ü,\k£?=VF£Sà?$bJ¥©Í?ïÜùY¶?en¢Äi?8ïŠ<N?.eáS®u‡?phÕôï?d.Î+gþê?ïÂQãïËw?®õ}›cU?H:ú¿Y?Zßr߸»?{Ó&¶SµÉ?}bùÞù(?ïœÕÂÙr¼?‹õóøæ?c÷ˆË?p`JŸÕ*?ƒãJ€Â^:?}Úf¾§ýT?ï÷jôõ'?A½ºÚâ²8? ÅÇ&?F>yô?NT^å³Ô?@s%õQÛHAGN4FGL J2203.6+6751?ш8U(rÝ@#ç@š$À:[¤ˆ
%À;ÚVų-@å‹
µ'@—Ö›'§æ?Ï"¸ß/%?Ç¥ÚZ)O?ù Äeõþ@5àŽ5?íõ«gᑿèÿ|'1ž¿èсèM¿é¾x`¹Ô"¿ïö¡÷6-¿êÐØËЯAGNbcuLQAC 330+067?é'ÁY?ü?Ç¡>Ô|?ˆÖšð €W?ꂍ¶ÿ?ÉӐëöÚ?ÇÖîÜ?éŽü›'¹?ÂÀÉ֚£?¢å$"ó?À? ÁËÔ¾0?Å
ć·w"?À Í6?êäÖ
4¾E?¦Ùq9ÂÞ%?¡»ã¤ãKU?"î
á«[W?¿û]ÄV[¬?£ÃS(%u÷?ê•ö˜
R?"óbˆ—Zþ?§s=˜ü?ÎöU+ài?¿–°×´îp?Ëéwþ>_?åДïvÆ?Ä6»Â¨ˆ?KZîþ?'Á?G`K?Ҏ*,¬å?Ä9kµÊk?á\¬íî[?ÌAz,ۚ	?·‰—J·Ñ?µ2oðÞ?×dA÷#ëö?Ë;3$ùW?å	ïk÷ä—?°ýl±;ô8?µMØ8p•?¢¶ÇØÀLÁ?И«~+?­¨ød¾ü?â¶aË÷åª?¦Z>f¢^U?»…›5 Ú? Ü·F%?Ó±Õ¡Bìu?¥Ezµ29TAGN4FGL J2204.3+0438¿Ñ°ÃáZ'7ÀCT!BoçÀ:
,·îïÀ<Qé{Y<²@ÖIGF»{@­|ÀDÿ?»"žñ-?¿ÆÕfú5?þ`Î\‹@Íêæßó¿ãӕ:a%¿âôÇÝÏ©v¿ãiÇåv¿çôÓ˜A¿æZ1¿•¬¥¿ænnD—àAGNbll3FGL J2204.4+04394C +04.77?ï±~È*?°@Y–D0¤?B-æ€o¬?9*Ī7?'}pº'Ÿ?°B8E'ƒ?撚‹€?†}¨¶èÀæ?[‰Öf??n¾qFì†ý?'ꄆuš?€:S»ü^x?ï¢d#ɑb?vu7'öæ?Z4ñô]b?Vbà"$?" tÿƒE×?tÝͱgVQ?ùúWu?e]Ñfï^+?g:ñ¤ç»D?FóeÓµâÒ?ˆb$?c¯ॴ¿?ïk2²!¶?¬âEÚÕ¤?aÝ8û(:Á?[´í«g=ü?^ ¶qÖ?¬ä{ØÅr?îäÄHL}?Ÿ%YjzSK?lºõÌÚÀ?v
pÈk«?ŸÐ5õ¾?œ¸¯¶ì†?ï,Ay?Žc‹ùDX?lôCÚ"8?hÚ0Úà®#?–áoch™Â?‹þÀȄ)?î£zý]t‹?…AN kÒ®?8|ÒpF*?hPíÙ6èt?¡z0ñÛC?ƒ\"zÔéAGN4FGL J2204.5+3634?Í9\ÇEHÀ.\ÌîZ¼À; È1\™^À<J'Œ"Þ!@ <7"À@§äRµ?ÅÑY¹Ú¬´¿£§àYF˜?â"Jb#á‡@+
s†	š¿ç|'ݽµÙ?ï·õÿËþ¿èÉ[]ô§Ý¿ås]û]Ùпãõ
}ìêÏ¿œkÊÃ!?AGNbllMG3 J220423+3632?ï¾è¬ã?w-z	üñ?@¥©YãY?2róV:?~àÄ[#9.?vw‡·¡é?ïÌ©ÒÝï?y[ý:«ˆ?DˆoÞöð?PCždÁ`?w½G?wü C䨮?ï?ç–Ò"ã?…ž¸J0f)?c#›¤*~?_‹¹es˜š?• H¬¹~^?"÷ïÙ±?ïW8ºË\N?pЖ:Q{?ZÃrƒD¶?ATxo(ßú?"w¬i<õù?p Óæl¿?ïo¸y¦×?…éI|˜#o?S™¶FæÕË?Fçg+£4?Ïb2·þ®?…5tY'Î?ïjŸq¯g?—™+ø?b[#dx˜u?vÈvi&¨?`¹'ë?••GH•¥V?î~^ýçKÿ?"C"ÑÏ?oö‰j?eïè!fS?¦§•Ó?'$`:04?í÷¦Þ.Q«?'xÕÍÔ%?qÓÄByŸ?c‹}P¨"?®K'ž
ø?'§¯È4U«AGN4FGL J2205.0+7432?çî0Ïå@.dvò¥¤jÀ:å*Óa,À<ap9N@xs²Ì›@ùš‹1!?ßš"Ñ
Ÿ?è…ë1;â.@l Ÿ²¸O@¢ÊšÃe¿ï}Ë<©Ôz?ïÿ÷œ"/¥¿ÎI‡9£¿é1ÿŒ<¹Å¿ìËÃAe%?܂›üu¼AGNbcuS5 2205+74?ìX)LT—\?ÃP\š¤u?»"Ç™Bló?Ã%Q#Å=H?z®àc9® ?‡µ†–#ñ¶?ëa´¤ÑŸß?ÓSØ!ó"?·B¿TT›,?ÀN`¾º?«_7
¬g²?«r¦c(+?êijV#çÖ?­¿kL¾7?²–«Mð$ ?¡Šÿÿ¢C?º'©5?¦+½‹gÖ?ëâh´»?¥õu"ñæ?¶€.àÿcí?ž2Çs3¸Æ?¤ÙúEëm?›çYnoð	?è´MùC^‹?ÈÌPlUû?Ìv2Óç@?ÈÑ£mǝ?wÃbö¤?€æaӗ‡À?å:aáOu?ÎÁëùžù?Ì6´Kerå?Ë4>r_!?½¿ˆ^¼V'?·ƒÛýæL?éN£íì"M?®\…Ú"Ši?³=Á¿n
¦?¢ÆË9¦t0?Á&gLÑ{?¨,u^8á?âÅ´³.Ó?¾€cR4Ö!?Ð}ªŽ-Ø?½"í÷ú?ÃíØÿk†?ºÕg÷œ?wAGN4FGL J2206.8-0032¿ïH3®`ْÀE4Áü28À9Lå".(1À<ºß%•@r=Ô¡ØW@?› 'W?±g¨A
wž?³¯—‡Æˆe@šfH3u@c,°ã?ßüÒ¹u×ó¿ÜÛëc:âÕ¿äa~õÿK¿àA¨a2Ÿå¿í'C¿rq7?·ð©Jç…AGNbll3FGL J2206.9-0031PMN J2206-0031?ï萪)+??U^øåUÃû?8±+YÅ?)©\à[Qž?dY0FéyN?S¥Œãð?ïߢõ¸ÔG?rM|¦iï±?>æ4îòV?Pâ°IÃrM?lœ'žH?n²;ÆR§?ïR˜ïXF?©'ùe©t?…NünN\ò?‹ZNª"¢?†0Rkõ¬?^t¡/ï–?ïÜM?P­]ƒX=?Gk	¿é&?.é Ö¿]Ü?mØ,Ã׬Œ?NVoðÃb;?ïؾÅço?cIVÚÝÿ¡?Fµ0qMí±?7ՃÚ'¼õ?pÊY†€KŽ?a؎´Ô¬—?ï æ.óˆx?ˆ÷ŒµEÐ?PZó ‡?cÒIü\ä0?…ųþÊ Î?…÷Ós "Ç?ïȵ¥?'ÅÀ%!`?‹3á
^}Þ?Œ÷;ÜA6?',øÙšh?‡CÐ(:Ër?ïžØUž\?qcÚöQD²?`"úÄpùŽ?P¸Az3?"$¿­Í~´?n-±ÖNAGN4FGL J2207.0+3607?¸+ßç¸À/°ÿŸ‡ðÀ;i£ÙŽÀ<c…Ò<xV@ 3
ž¤@IsÙìp?ɪ+¢› ?ž(Û@'üõ?Ö¡sÕB<@úm‡	¿ï¨P!ӏ?ëU°€æÅF¿â`‰ãC0׿éò"ý[
¿´t×~'¾D¿è '+"ØAGNbcu1RXS J220708.5+360935?ﮝÝK8?z:j¾ö"†?=ù—äî@¸?2"Y×R8?ƒh»øã"á?y‡²¢è?u?ïÊ^UuÓA?~'m͟ÅØ?C±÷ñé£l?KzNùüÆ?xZ–LÓ°P?|þilÒ?ï5i:Îw?ƒ>‹PâØ?dê¶-Ø70?b¥íö'k?–µãŒ°<?';‡'MG;?ïyÀoé"P?m2uë	
ô?IuOŽ·?8@ ۅŠä?øÌ b?mT'B!ë?ïS™ºÑ¢Ÿ?Šýqσ?Qì—ñ¸dl?E"^àG?"mÿõÔ?Ša~¶n…|?ïg˜J헦? Np<Õ©?T±>/÷M¯?c©a¡§Mk?'Á⺪f?ŸP¬EÛ}?î.À#é`¤?˜`5Êîú?qíylçm?kYù,H?ªÖN—üT?—òç!",?îf-4QÒl?ŒJoˆûœ?aEo]tg?\¶'ÆwÛõ?¨ˆÕȑ,L?‹òàMVKÆAGN4FGL J2207.1+4316?펙•Š7ÉÀ$FÎô©‹À:"qDúÀ<	Ÿ)üRÌ@ ¡™Ê–çŽ?ûèQÃA2Ð?ǯI™§"?ÐÐÉ<qu@v.	þ†ƒ@	n(Ãm¨¿ï²¾™-c?ç'!þW‰T¿áeHŽå
±¿Ù¤þývŽ¿Ó-eÿ8Yä¿ïÿäë8AGNbcu87GB 220504.7+430144?ï>{CÿD?"@(…ÜÙ?UàÃ?˜ê?R÷ÊáÁú¬?–Ò‹F¨WŽ?"spüF«ï?ïdÒxÄs?ÆèId~Ù?G¿˜ðõö?XžKç3.?'§´–‡«?2wœOɚ?í[ßµeZ«?¡ØÜ

'=?ŠK¾¾mî®?‹‹C+D?±×Š{OžÒ?žÂـz¾×?î×¥K‡š?wôñIÿá?lT×);r{?Qn˜ƒ«Ûå? À]ÑâùC?u¿Kn½?î
…â‹.?«4á´'˜?mAæjZÏH?gvÕy˜V?­Zé7j7?ª\ãÞEÌç?îHÙÄh5…?²X‹õ¾žç?agÕ×VvV?pðhC?ª[æ]QÎ?²6¿]79?ê"!ñ¨‹?¬ãÚû ¸«?ˆ€»®?"qfY,?o?Äþh6†`?©µ	ßî5Õ?íO8Ýõœ­?'õÊ`–}?|Ü´¾é€Q?láRE8.?³¸mê'?'èΡAGN4FGL J2207.5-5346?éê½ÑÀHóþ®û+À9yÝ÷vÅÀ<j'¨
У@oPk'kT@P.Ë?«¢•Ûc?žù
¦z ?íã™BÞç@§¶š0m[¿Ú˜Ïö¿â[ýÂ8T¿æ¼ìOIo¿å—,×Ï_¿êú³fÊ9¿ÎƘ*XÄAGNfsrq3FGL J2207.8-5345PKS 2204-54?ïðmDZ"?q«ülÕoÎ?4kYcÞÝ9?IúÒ=émõ?Z
¡Z_rX?mKâ?ïév›_8í?ivì Ê,ä?35¬ç¾?Côuó߶E?d"¯_šn?eýN4?q‹?ﱛ¯?zâáæEn?Vc"'L& ?[ãø€	p±?€ÌÍl:«ï?y þ®t·?ïù–d0N?.¶ŸÎ{?+u}†0$1?¼dFâø?BÉä~ÜV?(bòÞ{Ê?ïÏ7xgDÞ?~{óc3ú?Hàì,[?M»ÔaSž?u`gÑLò£?{ë"^â×?ï¼ô	§ž•?ƒÆí%æü?@¦¯ÓÅc_?SM{{#÷Q?q%Kõ½?'*f‰¸'=?ïi|ú®?Š%%Ƥo?^‡Õ"¨Ý	?a	÷FfJ?çò ¤ƒ`?ˆêggmLŠ?ïð~šß?L`©¬—é7?B[«24@½?5P·§?VÇ-QK?E³Ò4UAGN4FGL J2207.6+0053?ÕŽ]ëÀD×ú~¶¿DÀ:±Öv™ºQÀ<Uq€Ø@æ«͏À@ÂCÜ΢?ÄàĦbªÅ?¢ñ·¤ã–?ÝeêÕÌP@â«¡.
"?ïîÎ_¢¿ç0Èè#¿æfA¬Ž¿ê}ÅB"пÊX‰m~¿ïÿwD;ÏAGNbcuPMN J2207+0052?ïÀ€‹€§/?²®ú¾?DCïG8â?BÐ;W#ò
?}<±¯å‰P?€ã{!JÞº?ï¿r'§º?{¿ú«©"æ?LÏ5Wß3?U{Áp8ÿP?|­LNǕ?x3~ýÌø?ïd¼:Zš?"ý	B®W??W1:ëb?FstÅÍ?'ö»?"ÎáÇR0ò?ïÒ?啒ñ?U5ÞµŠÂb?2l(†'À? $šï#?u¹J΀7:?T¥u®w‰?ï	³ÖdXÎ?¡×/ÚÁµ ?_'D vã ?\ééîG?œÐ`îñ?¡SŸÂÜÀ?ï`¤…'i?x3Èxb?UI5я©}?`ñ/s;B?'©xjÂM?ŽÚÎìWn¶?îÃsH]M?"óԎè/?f÷uÞL¨¯?e-
W4r?¢YTFc?"r°[-÷U?ïl›F—éì?ul˲w?L¼q0›r?Borǯ¶?'†³›Ÿïy?tÙ`ödF¹AGN4FGL J2208.1-4507?ߒ'+·ýÀJ|ÁÁÖυÀ;É7PÏ%mÀ<òrâu«~@!ï0ì\?ü"þ_
?ßÓp?ƒ"µ?ªW[AÖJ`?ù²v‡›À:¿ïÿæ4|ßO?ïüv¨ÓÉ@¿ÐeºD	Y¿Ú::c~)§¿Ü˜bŒè¿ïïM•µ‹AGNbcuPMN J2208-4509?ïÞÛ̳¼?…à7Ô%Þ@?%'ÂÆ´¬I?$†å¸¨_?oÌ ÕK?…Ïêù–Ð?ïÊ:›SÐY?v1µþ{¥?HWgøðö?Rp†Û½ß¬?wàÇQtÿ?s^U֟e?îä]•1€?'Ý/VÀè#?o;ÂøZh°?w̲ԈÂÚ?ŸŒÕSÖè?'^7zÞ?ïs‹nøJ?ret‡g?PëÖOôß6?>/Îý0?ÔÀní	?rM{Ž¹½6?ïÊÌÙa?"ä@â?6Žüv3V?2þa/Üm?y¾ËX¡?ƒØ׉̗}?ïu21´
½?]M'lõ-?U‡™æhMË?d({œ-?@$á˜?‹X*"%"«?îqIƒN ?˜(bÏÌê&?lƒõ–c9ü?s5ðmz%?§#(tÏpý?—bðÚ
­?îŌDOô?ŽïêV?Rœ™YÔñØ?\6µcF×?£Vñ]¸³?Žu®c¨AGN4FGL J2208.2+0350¿Óˆ–%Š—ãÀCõº² À;RӘ˜èšÀ<«ÏèàÿŠ@oŠD¼óf@ᇿ}?Ìb~dßӐ?¿¶œ´¬?òÞU‹Lϼ?í¥ð¼¸yü¿îÛ
F9 ?ïã>"¹…È¿à"ä0– Á¿ä!Fkõ ¿áz+ª¨µ–¿ïÿCaԆUAGNbllSDSS J220812.70+035304.6?ï¾TÜd?sGO­6äT?T2\°?Æ?U5'Š'?{É^gJ&?q†Æž®ƒ?î÷&•Éˆþ?› u7öŠ?~BzÌÃs?ˆ¥Œ¹XÉ?˜\"µ…?"=èeQ
?ï!üT­^ü?‰Nÿ»Ž@]?{Î[-¨MÊ?€pŒûì?"ÌޜVX?"Hõcƒ*í?ì‰áǟ€'?"Nœs¨>.?š{°™s*°?GD~²ª?µñ˜?'‹ ¬‰:›?ïzPçVÄe?…"Á·q¦?jGöiI?jxƒPa¬?ŠåE£ÿø>?ƒ-оaµ?ì¬r:kG?¸Uñâщ?™;+Åè"?¡šÙ¿âI/?´M£<ì«¡?³•WþÍ-£?î¬6Ù?"/0öì%Æ?Ï=næ1·?ƒGi±Ù†6? ÈÏ3¦Âï?Žì3àÑ=T?è
l…lïu?©.:y¶k?¨šQΟwä?–3º8kC?É£¹v6p³?¨ÖÄzc¯AGN4FGL J2209.4+4329?ïêuë‹÷À$h'­ÄÉÉÀ9ºÆîj¬À;›Wëy`>@˜%ä@|dý°šg?·¶ böð¿¨*£dÄ?ñ`ú@jµ§l@?än.¡©¡¿ènÓr'¿åHNöÞ¿é¼ÿ¿ã¡Ö^ÆßοÚÒÁÃÚ4êAGNbcuB3 2207+432?îú»ç'
?™/¤dL%‹?D¹g"UÜ|?:Àá+¡ÛT? [ëPU	?˜óÜoÒ×Æ?í,°ª='?²¹,Éç?a—Ó@cXN?i§eƒ
Ð?¶á#êí?²Ž¯\ñ¿î?î9)Jã?›µl¢¯[½?x…"ø÷­^?ytÅúH¤•?¬ºÏBt¤?šþ `[€?Á}°§?vÿòQ­?k}]ÊE¾è?LHÙL€?¢® !—?vEããLh?íÀÏ4þ\?¯Ö±ÝE0…?_-ý®´æT?Vn¦WÁR³?·uA¥†?¯ˆJ¤¯p?é}þjÿ}N?Äz'Êl—¥?p)@¹)<?~¢¢'H»?Ɇ¼Oڑd?ÄQp]éÇ?ë?èÓ
 ?¬€Ñ7æ"?æ=Øl'?‡Š¨Ùh?Á!ûçJ?«qv"Cäè?ì5.< ¼›?"[è;Ƴ6?…¼ËÈ'&?q1Ä[Ù¬o?»žô¼äA?""æ kAƒAGN4FGL J2209.7-0451?ã뵊ˆQÀFÅ£~õ©À:aµÁŒäÀ<JO¾"4®@ âóÀ×v?þD¸)§™?·V3M÷ž¿¤"4áÅ=ž?îRàw¤|@ÕºåÈú¿ì¯©Ggž¿Ø†d¾E s¿ÏöN»ÏÏa¿çȧ¤WÚ¿Ô³çƒ?´æÐÙ÷­¡AGNbll3FGL J2209.8-0450NVSS J220941-045111?ïµg8{û?s§°åã\?Fœ<Á™?6'v
—ƒ?E€`å't?r駕ÜþÐ?ï¹ï{‰Ÿb?~­ý4ŽÉý?P+c±¼-?ZãJä¾ÿ¯?~ýipޙ¼?zªPb 4?ï22'¼»æ?†*}Òʯê?n̉àXå³?vlüí á>?•àf²Œ?'ÓcödÂÃ?îø³X"?|]
Ñ?Võl¶8?BҔž^Èü?ŸzKªá0*?|Zø'#D{?ïM¶ÿÛíÒ?ˆ[~鰁i?`þtéÄÿ?T&و?")^îÙÚ*?†ë«žÏšz?ïPÖöá9?XÎ'‰¿ƒ?[¦èDÌŸ?cÏ» sY;?"*²¡¡|œ?Œ¾´É/eG?îLJ&ù¶?"ëiŽòž.?wêO©¬Q?wL|4úÍ­?¨>Hóu?"aàœlŗ?ìèÞQô-S?›çMA(?m'…âÒj?eÁ¸!:'?·ÌùB䐕?œpOëAGN4FGL J2209.8-5028?Ý,›úqö'ÀIƘÀ¤ À;Lï͂Õ2À<¤u‰ïØk@ÖÙyÙ_Ø@œ÷S½?ÐÉý·{W?±äØfÌh?ã´£
[£•@Úºch°?í«ñŠò6ê¿álÓu]¿æÂIá nu¿ßmA£¹X¿ë®Íb¿ï÷9R1%<AGNbcuPMN J2210-5030?ïå¯]¸ ?dtLO†Gz?;vsõ+½?7«ÊJ´]?fâ(C‹ ?bX~¤|?ïÒtÜËÈk?p)SóÚª?DVa7ÆY?O|'%…Î5?t:ÅvµÊ˜?kDz©w†Â?ï—Æ!Ú<Ä?€GjŽ{?V¡Wû×ã¿?KP­–ªDu?‡:L~Ÿ"?€'Ùg(?ï͔¦sOa?UPRB`?D:¼c·ˆÊ?)u¹§|ÿì?v®UOª¯?TŸ&y!6?ï²û±LúÁ?|CT8?Q¡³žDzŒ?Lœ®OO¥?Ý=p>{?|¨«b(ß?3êX?ŠXexo?RÏ,ý|×?a7++ýà?‹¹ƒÄi?‡àAw-Xà?ï5´¦:g?Œ(ç/¨e?cäÐæî$K?lâOmÃ?–ßoSÚN"?‹:Q»hß?ïpà–
÷]?t‡'¯ä?VõÒ¶5þŠ?Cÿ¸ÖwzÉ?t Ý^?t9ؾp‡2AGN4FGL J2210.8+3203?ì'p Ú‰,À3Í_™Ã‹À;ÜjžÚK;À<ߧ[#<E@$œ^o÷à?÷&ª>,‹y?ѾÇüX€ ?ÂZ<¡ñ×É?ñÑU¡Îò@"ì3D{¿ïÿÿÊPË?æ´yï°&¤¿µ"¦:'ÌF?ïþŒÝôgp¿âüvÄ¿Ìp÷äÓ~ÃAGNbcu1RXS J221058.3+320327?ïaÇÀ?íù?§éWÛ©Ì|?5¬&K±°?6	-·¶?"pWbٓ?§Ý k«*Ù?ï¹V]"Ào?•–Z«åO?HúÊ_Ð?ZËBGu?€(v¾8º{?"­nOÎPY?ê@ÄßjÅ?³)Ëæ©ßæ?p¦Ãbe±Ó?LÏ~'^?Æw¹w&õZ?³K*úQÍ?ïajÙñ+/?@Ë#`̃?ZǤځ?QÅv׈¢?'&*t
g?€ËM°êž?ï­5³ž±?'"ФÞ÷?Fð÷Ñ#Ux?RÜo·²Ü?ƒCƒ¥u÷§?'ôò~äÁÉ?ïm8ß^c§?žñNw·f?`!¥T¸?w¦¿½‡Äâ?TÁ ¼Ñ?.
Ð\?ì˜%¼q?§3j;÷Â?hªo¯Ú0Š?xU2Ú¦?¹%ëW¬ƒ9?§&ŽíÀ¤?î*]FW'Y?*Ãë*E?xYUs/e´?z†5:&É?ªOïH²?œÄr±ŠÒAGN4FGL J2211.0-0003?¤üßp/ÁMÀEy¥q"À:ÆîᵒÀ<tÌežÀ@ ZS6Ñù?ýP"{rg&?ÊXyÿ…V?»?äq"&Á?óÂíÖ1Ð]@Òì؅è?ïÕ1U¡Ï¿æŸÿ®—¿Ý‰9"ÛòZ¿ã^M"0ÉÌ¿ÂaÉɍ'E¿ç]Ä×5AGNbllRX J2211.1-0003?ïY˜%¹š?®Y,°ÑÞ?Lšd"Ã|=?k¬÷®C"?"è*¾sz?¬_D›£P?ï•É¨!"?"ÅÑ´Qѐ?`?v€
?eJist¶r?†}¸uNw?3§,V6?ï1úO«¨ª?"×KMR»†?l[pcGQ"?v"CªNÉ?–5Gö¾×¤?'rK'—ÝÐ?î­ß:§_š?}08¾u¹›?]"]ZV??F|> m:?¤8ùpĹ-?|DòÂ?îÜQšQzq?¦–ÐÓ¡æ
?`3J,?~.½ÅUY®?¡9%Ö&³?£BxÞS«û?ïˆÏœàÌ?"˴׊+m?elɋ0–'?pØ6ŽºŸ?›áLÓÆ¥¼?"<_áúÌÞ?îHµ±°Å8?˜Pˆ+þ¤?pçÊ̼?qf"ö€'?©s"¨<Kj?—QѪ
L?ì¼´¦»@?šœ5ã?p,¾P½o¨?cû6?¾'Nt=zÆ?š‹tkÇ*AGN4FGL J2211.2-1325?⟝1Ý%hÀIÌ>1"÷À:ŽŸj"óÀ<U¢šÊB@§"å¡ì@™f`‡)U?ºöÄBÃ<?¨æª"xu?ßÁ6+57ð@Ó1p:z¥¿ÄnÖ·Ý&Œ¿ã[	pÂ	û¿ê֛'§å¿ç‰âÂW}ë¿ïÿåþÌú?ïÿ}Ž¡AGNbcuPKS 2208-137?ïÀvO	?´í–žäód?`2Û|†ö?•Õ[4Û´.?w«jÔ¥ë?¯ÕëØ¡Yf?ïä
šŒ!¦?oR\Iú?87¶f•P?KÑÝÃ÷ç?hëlÿîqg?jT–:­?ï» ô›Œ¨?t¸¼£¢š"?X#_a?L•@Ÿr»È?|&ÁDÌ?t-j¶s?ï÷;¤'#?4`È	b?)Ü*$Ÿ¹?ó6sç£?Lšfm§3D?2D6̳¿Ã?ïÙÛ²)¹?­Û5á²cÊ?R"+˜Ã‡?†`Ý´}Tý?m"àÕ@?¨Cß/À³?ï¨t­žU¸?‰Ä}ìì‡:?H»%x›ã?^òGvßIð?"W"E¹{?‡eÀ"©F•?ï—;qVk?y±:är¨?`÷XS¸•±?`JðˆÐˆî?…ümk÷?w¥vȏu†?ïäý¿uC?UÚ.´Ç;?E‰s)ڔ?8gÇiR€^?e »xD?S	
É:OAGN4FGL J2211.4-7040?Ú\®j͛ÀD~	VÀÖõÀ:÷Óc¿ÂùÀ<À!ˆæÃï@Šˆ¯'@¢P¨­?½¬/ô9xG¿¨•Ú¦‰¨?ìUÐììýÅ?þ•'¦8
Ž¿àr·B!À¿à-YÕ^kƿ剀Fâ<¡¿ã¿ÕØå	¿à­á¥!¿Û¡œ1úNAGNbll3FGL J2212.3-7039PMN J2211-7039?ïݏ"Õ\
?a)— vE?C©hÑöp?2,#²˜¤±?m†ؙÏi?`j•!ö,?ï¨VBNP'?{0cH}?Th…+Ðô?Xyí~Žå?ƒ]^Õg6?wµak=ÝO?ïtØ"Û ?zEï­µJô?dá+ž%Z?dœ×!°<?Ä?óV‰?w¹N²>ýÔ?(?mVvāsŽ?bc}Ãò(?FŒñaJˆ?ŠúÁJÆI?mÒ»V‰JÖ?ï±,Räœ?pj.n"¶ ?[;qŠLÆ?N5—V\?€RD!g?mXO%•?ïA«Æí»?•"!ُ@?b饯Q?h½¡¹¶3?›Z§N4¬µ?"óÌö%QA?ïBìäšI?†FË7î¦3?lšYC¦eŠ?g›Á¨§C?™dWB‡'?"ÉÄb3ì?î_z—{?Ÿ¸Ñôþ?}:ŒlÚ#Å?lÔ3ð.¾?¦a
Œ°"?±áÌÔ¨AGN4FGL J2212.0+2356?ëçÄRˆlÀ:q£±JÀ96ÁU FÀ;㶇*@´¸­@óŠ§ß­?¬ç…›ñô¶?¸É»{Eq@Á _ò@Ó/m¬¿Åº™™n¦|¿Ý7zU0³ý¿âÉUÐ-¿ä×àŠ"(¿æQßp¾Y¿à—àýy½AGNfsrq3FGL J2212.0+2355PKS 2209+236?íï¨M«H\?¤Tçˆ[?x¸_çÎN?oóYÁvß.?­îo(¿­N?£K^c'Ào?íM¨úà†h?³¼Z·!8?¤1ÝH  Õ?«õ$tJ?¦ó"Ÿª¬?¡)BZp@?ë'>°G?©²IÉ	º7?£ªû/?–…'%ª?½EHÒ)ó?¦ññ"Ü<Æ?ìlîÚÇ??íM|³Ðj?¡ï•6£ú?}Îû§ˆ÷?³¨
ù?‹í¾]>¹?ê¼'8\?¹±Ö¯Ø(?Œ÷=²¿º¨?€ñB뿃?Ã@uÞJðá?¸!bú¤?èí1"ú½?ÁÉTýÞ<·?¹_ŒW'·?¸Þ_f—äŽ?¾ùO(˜a?´÷-'öé?è5×ö ® ?±–¥»"TÜ?¬yIG—?Ÿ³É†÷J?È
Mߏzº?°DºXÑ´Z?职eº«?¥»¿^O@°?²S£‹_ð?•όúâ¥?ÄÏü¤x<I?¡Yž.Ž9½AGN4FGL J2212.2-7251¿ïgŽð{Ü"ÀCËØà†8À:ùÊd<À{À<"+¯±3@ˆºÏa@¦T…"RX?Ðkcü(Úë?¶å¸åº/?é¢Nt@fãr«™ ¿çò/ýô¿æ\°ožôL¿ä–_'‹¿ç!·à¬~¿ìì¿B ¿ïÿA(¿;ëAGNbcuPMN J2211-7249?ïȧfêMo?n•=xÊÚ?Sè­ýv‡J?I4&A@
Í?v²!ì'Ï?jՋ\qõV?ïéý
¾?"-½Šˆ]?X§HÑyˆ™?^‹M¤l<.?…pÔâ¡\?ÿ"]ê:Í?ïI]ˆ‹;?"eÂòleL?kÝÅüdÇ?k%¸×è€Ó?"X®Õ±pý?'­Wš#_ß?ï–Bœ²¨´?g&4ŸÕTÿ?ZÆÐ-XQ??F3õÐ'?‡~Îeså?e¿x±°§S?ïq/Ùó?†I#×Âìq?d+«ñÁ?ZDŠµ,r?Ž±I:eê[?"ù~Ò0†?îÑ®sùÕw?¤›ƒbLZ´?jÒLVÏ:?x§ŸKtDŽ?¡7ôÞ¼?¢ë€b>á?îš¼¯HX?Ž¦P"L·?vMìÅ?t†…H`?¡–±Ùi?‹¦¯rB€?îΕƒy5?…Œ
ŒQÿÉ?n½;«@üÆ?]0žÛYKÛ?¡*Ô|Ø:?"ƒÚÛýCAGN4FGL J2212.6+2800¿î*0•Ÿ#À6ülü'œþÀ9ëÕYcH¥À<O'h˜p@™õ *­S@ãøÀpø?¶t·7_?³ÛÙÚý<+?üüYÒÚ-@X±G
V?ïäC '?à¡
+a­š¿áÑ0ߛÜj¿ã•"ÁËçÊ¿ßÛڜCB¿ådÏÝùDûAGNbll3FGL J2212.6+2801MG3 J221240+2759?ï«ùfÅ?o¥|IOEã?TNã¶õÕB?Aø"»´Ì?'–\Оê?máNs
?ïwøypPÂ?Šwç1æ`?kÞç²þXÚ?pUٔÉÁ?‹
'µÌa4?…œJžÀ½"?ï"v«")(?‰k†œøÚÙ?x"3-râ?z'@Qüçe?•Œ¿ŠmL?ƒî3KÉ?îrn°?€ý?"_~¥?Z°Ôy}?rR¿/š›? «¼•sÏn?xÝèèߊ?ï¾n1®E?¬áÅêEÞ¥?p	&ð«?a2{vǞA?šð'¡C6?¬â]!¬¼?î‰2ìfp!?£Š€€ÓV?'fŠßP·Å?'~3åõ7±?¢Ó.'ø¬õ?ïÖ{È'?î6LW¶?–"ëÈ̞:?‰­ÁžåA?"¢{K˜]?¦Yf€I?'³£ÇJí?ì<_@Ï ^?™e£NÍc8?£Bõó©Z?îb¢¨'?´{Šÿ#Ác?'ø¤Ÿ°jAGN4FGL J2212.8+0647?êõtYe™ÀCfƒ#5.À9ÒÏr™zÀ;Ø£'@ßÄ@/1ÜF‡@m«w?¾fLæ¹Í?Ãx~‹ì@'pŽ@ÕO¨3æ?Ӝ=bá÷¿âS	AÈ!l¿ãܸ2¿êÊ©ÂÉn¿éö•žoû¿ïþ-͘¤§AGNfsrq1FGL J2212.9+0654TXS 2210+065?ï¼/[ÀΚ?x†]Ñ?fF2<³Ò?fvÐä+³?vÅ9Üql?}åÐ7f!á?ïc°žÃÏù?ˆEG²i?lÑR™†™?jìhº?ßƒ™ä(o?ƒÅ0íÑÞ¾?ïBå씤y?‰J{Šv!V?rÙ<|Ê	[?rŒãÏ?'ìóL­›?†t(hKeQ?îD¯Ecš?}Җv2¼?ƒÔÑÇ<"ô?ai&Jô›J?¦¿×:ÌË?yÛ¯	3­œ?îÞ￯?šEŒâkM?'¤7m¯¤×?2"³Èó8?'}äýÞ!:?Ž-W`•ë?î!Ù­l?¦˜2úÙ?†(+×Åt?"àfH
©Å?¨d×o7ý:?Ÿ›N+…?îÊÚDž?óÀĐD/?'Ô7üK?ŽÐD€¬pˆ?§mù?·õ?—˙ò"?ëŽz5ž?–Η£gÝ?™##U —?€3üFæ?½Cf`uûI?":¢öâ
|AGN4FGL J2212.9-2526?˖[îà•NÀKHßÞøH|À9Æ÷ê‡È·À<f1ØÀ @©þÁ'…@DAãÐ'?µ_ý–™4?ÀT5¡Íoµ@áDS@fý5uWÆ?ïeç}R;¿Èô 8Y¸®¿äövŸ´'¿âŸb2Ô¿éKòJ·¿ïÿõž}.)AGNfsrq3FGL J2213.1-2532PKS 2210-25?ïð"cÐÚ?Nš›ÈË?6ë³ÒwA~?/ÛïÛк?Y<MIp¯?JZð$F3?ïæҘyð?kØD•RW|?79yQ?CMzw§ß ?g+/¯¡=?h´^™ý?韛Ï)Ñé?{|ÁSDê?fT96A½?tZ<ŠÚ@?ûÐÆV'?qS\^¥ö?ïÞKÊP='?K˜4öj?Þ?Qº©È"?4<š?›D?h×-,?ÅY?G§~ÇAþä?ïÝMi'?aòЕá™?Q/8jâ?Hû[‡Þ¦ú?jbà^ŸÕ?]&§û¯S?ïºw®žt±?:lÐÊE§?Fðþ£¶U™?[§ïOZ?æóò"?Ñ5	4Ò?ï{·¼vI?ƒ2¾6菘?nKë™t8j?tD'|©ÿ¯?‰!Ϧ?{öe'Ç!A?ﮑpUR˜?g•¡­._Û?eµ"Ñ,(5?Qy…&ká½?}ܶ}î«ä?c˜AiŒAGN4FGL J2213.5-4754¿é"ôTŒÀJƒ2a|ÚÀ;†¯²	ÓÀ<²§$œ—{@ ´-"¯¹?úèleƒè?Ð04:Å"ß?ÂîräÎ÷?ò"ÏÝù@'óƒðºé?ïû‹'™¿ìYÙ$Éã俵Ûc¾k`¿âc€4
¿ÃÇT}ZÉ¥¿æí¦a(9AGNbll3FGL J2213.6-4755SUMSS J221330-475426?ïži_jÖ?ˆŽê}"ß?CîQ5õ
z?:/b#XK?‡&Ãaÿ8?ˆ)˜í±¥¨?ïµ	™©?€a*hœ"?SÁ\EÄ?\Dš–ž,p?€@O'Ÿ"!?{ÌVîL?î×¥°ÿí?¡°"\îÃ?\žŒ¾Ûðœ?YñƬ£?¡ °‰&-1?iËQ Ò5?ï;ø	Ui?snŠgƏ{?D|ïC_V?1yIå]˜?—ÝÅ>K?s3¼âX?ï
¤"ü)d?šå>—æ?]"*&æ
?TØúHÙ'?œyJÚôÌ©?šjoƒ8H?ïIwüð½?"ßð??F?_WGûÇU!?n9ÊN´Ã=?"Û«%ÌÝ?"3/
Pú?í›nÅId'?-Gr­?`Î[³›S?^ßqïnö?²ž"iK?œì¼'úJ'?íÆÚQðœ?'±®åæa9?Q±Ñ÷š‹?G.ž²Ù
?±'f(&Zu?'˜û`ŸW=AGN4FGL J2213.9+5948c¿é¸a\€"i@½ZiÀ:ôÏJVÀ;N[`xæœ@É"
–ÜÑ@l¥³Û?еHŸ¸?ÀNL(Í~£?ö'SZ(@GMƒA?í#Ýàpm¦¿æ͕ŸŽü¿éÕÀ˜áä¿å|ßÿÚkF¿ä9AG`¿ïùÅôkwGAGNbcu1FGL J2214.5+5949TXS 2212+5958?ê†;`~Dÿ?¶,™'öˆ?ƒÌ–
!?": fu?ĪQ$^q?µ:•‹V°?âí=ê¢(?Ç]¡pÓ}?âÆòÞ"?¡ª1Šo7Ï?ØGWËv"?Å«YÕ´R?ç´ß­éÌ?­d‰Ü&é?š¹¬ ¿D!?1—-¬×&?ÍØNüùvŠ?«S5?ԋ›?æ1…›WVK?£ÔÁÖØ?zwʤÄê?nȐRÍ8?Ò±!N£ã?£ó:l‹º?ãàý-ÎÖ?Á÷" ³Ô®?0Õ/€ž?ŠAÿ֟!?×FK]in?ÁÁ–v,4Å?ÕÀFT€¾_?Ƹn%Ío	?§4«6r?±y6€MJê?㬒%µÙ?ÆVGÏb½?ÝKï-[2?µå>º:W?¬Õ¦=«'? Zãä1›?ß0–Áº~?´çš7â
?ÖÏLÝy©?«$¨åH?•£¸"é?‰Œý€©²?㫬ÚÐ+ã?¬´‰‹™!MIXED4FGL J2215.4+0544?á×~4Ês<ÀCý—€º¥ƒÀ:¯¬kbOÀ<ióB'[@^´¸ƒê†@†ƒd£î‡?Ärj@:­¦?´Eyܺր?ðé›9¬Éø@ár¤P¿ï«.ýn€;?ïÌÄ¿77û¿èê~eᆿԑMjÙ¿çÂ[úҙ•¿ÈNÕ:¯~]AGNbcuNVSS J221513+054454?ïͳí{÷?gBÔ¾™:?AJ¡2',C?/S€AI?vüãæýÏ?eþ'~2?ïÅ$wâj?wQmtmR?K¶j{š
[?Q–ï'—?yöö§Ë»G?ta'°*Ëø?ïwü×½§Ò?€KhMb/?_7¶Ä-‡?I¨ÀEiû?ŽÓHŽz‡?'¾Ȉ?ïQ
F'p?lÜɼÆs-?qªÉ:6?R«Ó"Ò^?'sªRÁœW?j£ë*# ´?ï›|­÷ä?|~$­™?S滏é
?F-Tö/Æ?†¤9¦VûÁ?zÌ°tô&?ï;.×ÙÆ/?"k‹¶¤cÄ?a+ò.?pNÑʐ?–tÄØÝD?',Âù?ïÐ$x¸×?Š~n"¥úÚ?jåèî½'?b|ËÃ8?œ)>ZEd?‰1öi ¥?îG©¢PLt?‡?Lç§S?…~lÌÄÚ´?q;‹›¥õŠ?¦%Ê©Ð?…½þ@?AGN4FGL J2215.4+6105¿®7Ðf_Z"@
ª:›À9æ†t"çŒÀ;edù~Ü@GK1¬ ]@øÍ ¯¢ð?ÌèæˆàŽÌ?Îü¿¿s@Õd¶býü@y-Å
5¹?îFÉ))?šg8ÚxBB¿çÄô'6ô‰¿æºÊ×)G!¿ï'>ˆPò¿ïíx:¤AAGNbcuNVSS J221507+610506?ÖþÎ+
‰‹?½É§~^ª°?œ1"ý?'¿ŠdµpÂ?ãŸÌҖn?¾ún=Ù-?ِ‹­6ž<?¿–pL÷³?½Û.Nò×N?®ü¥áC4?Þø¨¿«ñ?¿¿þ)³z
?á?Ö&4??²grËÿ'S?°?UUlÐ?—ñÇù–hé?Ù³¹¾°²î?±þREÿ?ÚaiÒV¤? p½!FU?ù…8IÙ¤?˜"MÃé_'?ÜÛú¼Š?ŸË;.'¦O?Çol@¯.?³§‡N*"Û?¬í0—Q? «¸z]!?èUQøè?¶Û®ÓzÄ?ÃìDÁûãf?¸7x2ì?ÇwP!34?½i" ç^Ò?å'Ç4:"?ÁÍ(qۇ?ÏÏIôë¤Ô?°#³'¼ô?··ÖX'FC? £¶­?''?å2·bWc?²&
f|?Åz)ÅSå8?š¸•)¿¹`?ÊûºsâXƒ?§Cì¦ÍX?ãâ†ñ²p'?§$m íKMIXED4FGL J2216.8+3103?ïûw%Œ'±À5Cú*ÓéÀ:'S"¾À<6­•Ïà~@êûRò\@¼¾´ .?Ê\#—^ÖÐ?Ìvh&¯í?þrÉä»@ÅR¥>hq¿­QƒD1w
¿Ùè:œ3&ô¿èï^&üĿ拃ŒÚ¿ïýŒÙT›¿ðAGNfsrqS3 2214+30?ïx"€ÞaË?'C)kU?}«"ƒ¼¦M?"sjøEÈ?ƒ!ΈA/?"ÏSƒÃk?ïDþ$Ç?Š7?{!9ôo?Ž"H?—ìùƈ™?ˆ×ùáí/?î-ÐçÓR<?—dqãé0?—ã3èü—?'p=l×uœ?¡1WŽLØx?íúQ¼Ì?î8¬Õi1%?~/¡ÿQØÝ?'k×<Ýîî?o´1"÷K²?£?GjAC?xãÛìF\?îæÊS9§°?œùÔ¬e?U>¾F±?'…é•X·ê?'ÑvÞ6_@?‹ò®!ª¹k?î
ÛïÄ7l?£k9¥aO°?/"#UH?'çã ñ2?§
vî¢I;?ŸÚ
€…Ç6?ìC‹ñ?¤ETh¥~?¤ãæ;U8
?˜8ٜ[C\?³u؉Äds?œÌN×çM¦?ëa§6à?˜›óï"w?¦ƒ%2ñBC?‹DĺzR?¹±5!"\?"Õ‹Y²EYAGN4FGL J2216.9+2421¿ÐÒZ?ÜÀ:r¥'ÛçóÀ9†B"ÏÞÀ<*4žm>@oâ~9ì¶@é©¿Š¯?²˜;J®Ïâ?¬uüº?ø·…Ýúòz@
°ÕöA:¿Ò}ÆUˏ¿á>Ÿ&Kn¿å–¢='¿ãh4çÌ-¿ãîª!üÿð¿ì…ΫÊÆAGNbll3FGL J2217.0+2421B2 2214+24B?ïñÛË©rf?KknA]ä©?'Š™0¢n?:]G`"Ñ?YW$ÅØJ?Io*_!Û?ïãÓÝY¯?m	6! Ž?7qݟ'¤C?D
Ùæô‹?isð1gÁY?iæ8fuB?ᆰþø?qì2ÒgüÌ?TWš}
¬š?T®Q	þ?{"šRio?q áKä?ï˚ï@Pc?T;²f¤¹°?Q<ã€Ûl)?0PoÿS#õ?uãOyq§S?R}5þD4'?ïÞÝäÏw?aΝçñé)?<Î֏«ë·?0,thÁ—
?mˆ@r¸6™?`\l6î?שּmõ?ƒ=ÁbP¤?HºpüŽñ?U½.è¬l|?ƒý®œ?'m)Yƒ¿"?ï–;Þ¨lp?w˗œ­?`?‰•Yá?Z#ž²1'Û?†a%ê`Á?uÚ*Q6ý6?ïvLÇ-ü?rgF_.¿~?g¦ª,›ŠÒ?PO"@¹ ?ŒŽÂ2çtH?pxbô¼AGN4FGL J2218.6+1941?Ù<®É£ïÖÀ>P;€AÀ:ß!5Ú­`À<L½}®'@˜o¢û@V	™Üµx?Î
	}Ø
?¶$ø¡«¥¥?âÙ`>.8ø@´4¥y!¿Íg³BW¿Û•=׿és¹jð8ã¿ám —d¶¿ïÿÚpú>?æÓó! 8ÅAGNbcuGALEXASC J221854.64+193841.6?ïÖ}£ca?f]^3¨9?J™ÌK›ú?A3PcžS{?qn8•dU?dšPl·¶?ï¤Ã§Æ>O?‡
1›ø?[ô#Æ^>¿?e[­4'?ƒP'•¤¤ˆ?|¨G½ôå?ïbwHXUÏ?~oîï²?kvhõvú?g¥ðaä»?BIΧP?z:áÒ4F?樂©<"ž?dgWfÛ?T½"RÛö?8¦cÂÞÐ*?ƒ¸q[B?cÅų/B?תּ©U"?xž¦rÔï?W€è³Kú?OCàà á	?­8"Š'ñ?vå6ñ›È¥?ïÿäí?—Ó¥'Æý°?gƨ]'1"?t˜ü:8?œ§.n¯:?•p'/Uê)?ù®Ø?Ž·´Î Ò?xxMBú¸°?u`óVïõ?¡(†¿žÒC?Š½yÆáŽ?îäÈlü?…‡Lýï?mþ³0çÑý?\He'ù4?Ÿ§(Œ¼?ƒ¸/üXëÓAGN4FGL J2219.2+1806¿ãr"'¿RÀ?¢i'ÄÀ8þÏ;<1À;×Q!ZÛ@¢ª‰Uÿ'@l@šú©?©¦"Ô¸Ôr?µh¯‰â@
¾cb¥ç†@"Êb9[¿Î"¤)•z¦¿Ýˬ;\Í`¿ãü& ûù
¿ã@/€ Kпè|·áƒ=7¿ìbíç$AGNfsrq3FGL J2219.2+1806MG1 J221916+1806?ï÷Q;ÿú?Am¹aK!¤?#aä9¢"?w…'Ÿ\?Mã"‰‡WN??Ìp
pó?ïìp¯H5,?eÇؓIßJ?.K ±L}?=½w%èËh?aªžMÁy?csXÈ/7ˆ?ï³¼3]·?uÚåÌ®µ?]á'µï?d="Tiâè?©³ÁÇ?rYÃúnF?ïøtö—ô?1éw¹©^s?--Q¨Ãº>÷ü+²Lb?L9U>ûW?1>b#Ì\4?ïî}&r¢?RìÊgC`?0ݔݠ¼g?(1ô©"—a?^ÎNµû9?Qfªßµ-Y?ïÂ6J-ºg?|¿tƺ³?C›`ɳŽ?XpV@´¿%?|qnï*Q"?€\›ÍS—ñ?™ùÞ?€éǞØ?d›ÊmÜ?dNù/$ßt?ˆ79—‹?{dMÎûµ?ïîïe—Î?Ot¹‹¿R¤?"Æ!ýD?|]d?`N"%"¶?N9uðÿˍAGN4FGL J2219.2-0342¿è®ËÆx°ýÀGfá`؇ìÀ9Ê©Hš¤À<*yØ32\@蹃ÄÆ@ôɅðoi?»Ë"?À. ý;)¢?ü6öl‡š@íèQ¸"k¿ÏX"¿åޗ¿æ·û"p=¿è§:¬Î*¿éÉc@—ë¿ë³@S'D¿íý}¿HÌAGNfsrqPKS 2216-03?ïøñ/¥¢?=Éä¬Ø)?'£É‰þqb?©P|¿(?FROã¾¢—?:¢Û·¡A"?ïá—Rӝ³?y'Ø)ÿ°2?9‹:  ÿÈ?T´hBÚ©-?k7EõC±?u#ÓkºÊª?ï¾·ÇhE?q°
CË^ö?Xd"Û~å?[Šݙ]ë?z‹—&Ä?p-¬d˜?ïé|f§Ì?Dž=¶ˆ!?;~_•µ‰? ÆÜR©?c¦n÷Öý?BÈÄC1þì?ïó¾<!"?Lg\û²ò?5ÍgûõÙ?1	]¡€[R?SA¬ Äõ?H¡)"î§?ïŸ_K"þÕ?Š¨ÿº¡+R?H|=ÕÉ?WÚ3À´T?†¦…\Ãë?‰‡Lñèhž?ï@äæbå?~4¢åkÖÈ?cžG?U?_ªE¦¹Ðä?‡È5¥Vä?zÏrî°ßs?ï¾ÓD¶v?gé$:ò±?U}?¶ñ9?Bµ¯/iY?{O~[è@–?e–ëy>:AGN4FGL J2220.5+2813?Úg»—žGÀ7ÝÀµgÀ:Dmî$À<z8Cƒã@ ÷X¼…?ÿ
ä)à¤?ÂÁòh½®¢?¥Ø£š¤\?ã¹
"BË?þ'ÒÐÇÙ?ïú{üР—¿è¬Ôÿ÷«¿ßd­ÿ'+¿¿ÜÆOo©Ü¿Øå$ýd¿æÄç=AGNbll3FGL J2220.3+2812RX J2220.4+2814?ï›mâfÎ?€éîâq‡Ö?HTȶ3A½?;Iõëdl?‡ŸoԈ?€Šî²¯ýû?﫸Ä=mZ?}CTĹ<?X`ðé^>T?aÐ%c1º?'°Í¡‹¼?x±4\ÕKR?ï_^¼Æ;Û?~·M(»­?bÁ'¿
õ?bºŸú?'¼q'¢0?{»XFð)Ë?îæZ	‹Å?së	†æ|?m"@yÃÁ…?M?Ý?ŸŠÌªÆ›8?s[Z="Q?ïR`z¡Ã?ÿ>¸B>M?Y°'ÆZ§?Kä+0pí?"ôWP*?G®'å?ïe+'öê?"E	Ñ8b	?bûåä׶?l_¡,ãF?™óÝá0×Å?"|£(^yû?îÃý9wC?ghBTPt?isÜ»–:?añûæ)ñ?¢/¥3P›k?Ìs3ôç-?ìïO;&œ¢?øÛA±Z"?'=fÂF«õ?k¾sЪ¥w?¶=ÙM"mt?×Äõ«ÎAGN4FGL J2221.5-5225?ß8çJ°ÀJ1	á*QãÀ9vvü¶ŸdÀ;ñžbeP@üDËaé?ù½R;66ô?°«¶ý'¢1?ºˆ©t
n@‹"ÞQZ@Öjˆ	#j?Ö\_ý@²ù?ËÙÂ~•1U¿Ó¹Ššù*¿Ó«<äâÃ.¿Þ Ý%	¤Ä¿ßÝD>HeAGNbll3FGL J2221.6-5225PMN J2221-5224?ïö‰¦ Tx?J'"ºO-M?- Êl?Û?#Ñá'O V?Nq4–¶P?HF£:ʱ¶?ïÝ؃gÍ?ql6T·?@êòO{?KÜßò¼?n"'x£$g?n$äy†e ?ﮏ4ÖR?wjäÙíŸf?`H®^‹"?cûEÔ/ç?€JK}ö´?tái—iWÎ?ïPª²-Ì?sÖS%Bb?XIófYR?<nz}TAú?"f
ˆà‡ì?rJñÀÍ=?ïër±Å¬¿?WDî£ý˜?@)® ið?4ƒ$8~‰k?`'ârL_ì?T×95¡d¤?ï¢W®Æ/,?†'kkÁ–¤?NÓ÷-‡ng?ZÚÞnóñ.?…|ÔÎ	I?"þqI>Cz?ï' fŽ?€±•M×fÀ?dkÕ
Õö?mwo³L4?†ÛB±./?|{|ÞÜô?î–ü6ØëO?‹9¿•Øî?eA¹šSE}?PþË4侧?¥< ö"d7?Šù\Âu´AGN4FGL J2221.9-3504¿ïÁ£n.±ÄÀLžÁ~ºñÀ:ÆùáØ͌À<§¾Ê«Š]@û±r(f|@}õÏ$•á?ÉìtÝÍ{?Î3†V¤?÷E¶ù%ñ+@­ÇÜMj?ïþ[Ï߿⿛L4¿çîYyîÙg¿ìîiÀ
 пøÌ?îÛ@Î&i AGNfsrq3FGL J2222.3-3500NVSS J222227-350942?ïðzhžFt?`Œh1ÛWõ?435‡'?D|UÉùÈ?Yþa¾ä?]ÁÙ󉡕?ïÁ8ô?€ïÄgŸ?W*¥T"«?gI-øäa?yfºWRïà?yð;)¶°?ïuÅOd?•pƒ!'_?sAðIÛi"?yÊ/–ÍÄ?› ËE›è?"0j"ãn?ïì)çZÍ?E¼p«Õ?:ádg[é?#ÚXyӊ?`yøP>?Cˆ
Ñÿ?ïå`jàò?lî#[:=ˆ?;–%LЂ¾?>ö#xSû<?g,Ðqµ¸~?kÞ֜OȒ?ïz ×?[N?"«7æF&?a8'ìƟ²?u•Jä܌S?	©wHt?Ñò%³‹?îSy—_¶?±†FìӜ?w«Ì|$?}Z–³Æ³?§Òû@ Ù?Ç­ýI"h?ï¸:§y^Ä?lzà3m}ú?UbAú²tm?Eð÷Cëd<?~Š°Xå?jЗÔ:ßAGN4FGL J2222.8+1209?ï¾îÕW­2ÀBWìÝ
Œ°À:c5*"8	À<8wškP±@¤ÔpZ0"@/MzÝð?ǜ
b.žN?Ł柆Ã?ü!¦ä÷·@T?b¿â½/k'–G¿áÎ耇yÜ¿åƒ) b`¿âя–n¿ïõ´yÒª¿ï}lÝxì{AGNbcuTXS 2220+119?ﺐ6ïUc?¯*]åx<?Vr›?t£?ƒèº"™?}=ÖÌÁ>?ª^ìö='Œ?ïÌÅhT}0?t,zSxŽ	?Ha(ØNÝ|?QFÈZZ-?v'&֝ùØ?qgö‰^¸ó?ï"ü§ìÿ®?"³Hîæ?hOm6Ï?nÞà¤Ц?ˆ¾Â'jB¸?'¨6~«?ïˆÛÃ6B?e‡p7¥§¨?c&0Ñd"H?FȂ#cŸƒ?ˆÿ«Ý™Ë?c‹ä_¸e?ïÑnCnX'?~wíص?S`àÿß?U™Ó²1å?r‡†J'?yº»ÓÚJø?ïWÌîcS?ŒÑ;^ŠUØ?\oGOc¯A?iÿÔ(€?"?mºSߌ?‰Ä€íƒÚ?ï5
EÓ¾?)e!`Ü?pµq¡ðÍ?s"Ëå#¦?•0úæéî?Š0º5…ã?îÄÙâ¶?"Jµ‹?w:Á]µ?dnA\,Úá? Ò:Šj|¡?'¥O}¿:AGN4FGL J2223.0+6746¿íÔ\B@!©Õ<ÝÖàÀ:~?Àà/€À;Ú@@aïß@dða|qÁ@K³ŸÕý?ÊÜøHр?½û
wÓ N?ò_V§¬Ô?ö"hëPñ_?ïî}†¸–¿ç6geiç$¿åý·³àm¿å  †Þ+¿ð?ïÿÿ)@k*AGNbcuTXS 2221+675?é.˜ö˜?Á@+Ԛ ¨?"UNÚç>S?§ê`‰=?ÈÝ=õÑJW?Àtð'^"‹?å1hˆ)¯§?Æ<Ù¥"cØ?¤ÇÂe¯v?¤ß '"ï9?Ó6¢ö±ð?Ä<>¡È´‡?ê0íó…j°?¨J	x«¯?¥WHNÃõ?˜M7wWÓ»?Áæßh°Ä?¤uÑ+jâ®?æ—68(îê?¦­Ïi[Ð?¥;JÒày?…×ߌ]?Ð**5ˆ¢ü?¤@#•26?åbH/ÕÂ?Åš[À·?£-`©#?¯ÓÚâIÊ?Óm5Ã0kÙ?Ä·Ûï)™?ÕåM
¹†8?Ì«ãV7?³®mÞw<?·ÑñY1?âc¬çmý?ËR5Ï<52?äö0K!f'?°^éîWÆ?²1tQ—"Š?ŸŠaÐüó‹?чBU T?®×Ò±¶?×vèyÑ}6?°È[àyȆ?´‰£
T?žà¾é…ß?áÂ:Žµÿ›?°v ïÜîÄMIXED4FGL J2223.3+0102¿çW1õÆk4ÀFMa€M˜9À;>Õ'åÀ<‹wI¹L@ Äkq=/?ü›Þ'׶5?Ñb
-€l?¿¶«G—?ñÞâ^.‰€@é£È¸?çÃ_›q
.¿çXÛch…%¿ãØMꣿÇÍ×0¨ê¿Ý·R<7馿Þ4hݏÖAGNbll3FGL J2223.3+0103SDSS J222329.56+010226.6?ïäƪ/$A?\X©L¤­?)êù6­°î?­d:Œ+?iš¦6n|¹?[ºÚ›êD>?ï«Ìå	?^«î.Ò?U"¢Ž–ª?[ó6ϐ°?'Zf8Ó5?zó•q?ï†pÄ'%£?røÛM·üƒ?WO®TÃÑþ?;U¸À·T?‹yÙ=|?r‹Q~ŒÖ?ï#ôZŸ!³?u]s>4Dà?R§Ÿ¹"Ï?9°¸eI›?šVúÁ/hV?tþÀò«†?ïÒf
1B~?eR4dh?:FLJ-F…?-Là
S–F?u(ŽPz•Â?d'¢ã¦úF?ïF*zc.µ?tîè¡,?]ÐEÔ}̱?gU.v†'K?•]¬Q®Ó¥?ŒCbÆÂÉH?ï0ã(?Œ?¨Uƒ›ÿ›?^Ó(õÚE?Kg±œ‹{?˜mÊ\$Ü?=©A
?í[ˆ³²
s?'߉–6ü?e6ñÇä‹?WH½½G-?´zÕ#[Å?'áòL-î	AGN4FGL J2223.4+5814¿æhO(v®?軈!!7ÞÀ9ƒÝòŽþ5À;'éÃ}˜²@ºµ ¶Cs@Ù¶3kg?ÌÜ9|Mƒl?Õâ‹ûÌ>²@é!S6ß?éðŽîoß·?ïûøi2Ɂ¿ãç—¾Vè¿çðSà&ñ±¿ï6©	y&¿ð?ðAGNbcuSSTSL2 J222330.04+581350.9?äkO«ôC?є^zù_A?²
¾¥Ë4?É+'²"?Ò¦ÛBþ¤®?ÎÂ=D␷?ÎÓ)â…#?Ëö° ò(|?À¼½]÷Š™?»tÌÇw?ä
ž	|?ÊĔ‡È?ábçR"üH?³å±`Ö°?¶ï¹"?¡ÛpT€ÿ¨?×~pmü1ê?²ÄWˆÀ?ų4¨Ü¶,?¥êÛ\+?Ì4-jWÝ?¬cÎPmqA?ã†'{2êþ?²ý
NÈ[?àßül%7?ÑUþø?¬â…͈)G?¾YûÁNa?Ú£¶m嶩?Ð~ñV]Éy?·P"Ó&¾?Á¦*1èìy?à ƸÐZ?îu^Pî/?èN§3úÈ"?ÇãüM\Ãê?ÖKþEÀ©~?³{=sûf?Á©ÝX$/?©5È$D?ào‰†3–?³BÝÞ«È?©ƒj&f%Œ?"€w²ß¨×?Ζ†‰ò\©?µøCgƒ¨ß?æÂ'»8ƒ]?·ŠŸ JðMIXED4FGL J2224.0-1127?ï!h€ÀJ­>'À;X"üS£À<m
Ø/×^@¹¡"I¦<?ýœ>	P
Ú?Ô38üö¶*?ØÀyJ]@4…]¢r†@Fg˜jš¿ê6ñL¿ëk»À5Ö¿Ò\rœª›¿Û×£TY¿é4ց+Ž¤¿ïV›LøWAGNbll3FGL J2224.6-1122PKS 2221-116?ï¥.Xì<?x q
jxU?^w1õf6?^k_jåÏB?'å}Ðì¾C?u$UeZ>?*œ`É?ƒkvm0	Q?a#ñº€?d}ìì‡:7?…,`ð«…?ú{#gYE?î÷ië¦?'~€¹xÝ?|^2ž¹m7?}ý씽5±?™û5ï9Ù÷?vÞ{oÖ?îd9QŸ×?ƒ Û³Ž?kûkÀË;B?RÜe9ŠL?§ü´+wD^?'¥vüɅ>?ï!ˆÝ£x"?Ž[…´JÐ?tÖßNqq?r þPð?–™,tBÁ?ŒgýÑbÅ?ïŸÞà©+?˜~î³×|a?n†n:c‡É?y¹åÏë?š›6U;@ª?•¯¨3AI?íô㢄ØJ?›¡Ó%í«?‰þåÿ!)?‡u'¼Šôá?ª2D Æh?˜)ɲNö?ëè˂8ð? "ªª(œ?xÂóh*«?jAÞ$¬Ä?¿-ƒ¾2w™?Ÿíð¹%ÑAGN4FGL J2224.3+7737¿àÁ¡ÕŸ¦›@1€¾×@ÄÀ:yôºQ À<Ó'¹¬@*CÜ΢@ˆE~R?Øb«{™Sy?ÜÓ¸#rué@ÊÊ¡yaì?ü¨pÄä &?â{à­Tb¿áʁ=­4¬¿é1G ¨"¿íè?÷g¿ãŽYÊv±¿ïÿÿ>¹úAGNbcuNVSS J222721+773319?ëâu/ya¸?¾ÔRýþÈó?£?dzñ?§ËMm\~û?·cRf:'Ä?·òmÕSV?ìñRͤ°p?µyº>ˆY‰?¢ôÖùmáý?¤
DŽ\D?­õü*Hþ?®p˦?ë(Lƒwz?§uÈ îø?­¹b¦'$!?tX¹á?·à꒺À ? ó¤¼uW?ìQž!'u?—‡xùž¹?™öÑ4
ïD?€ó!þ¶•?¶õZ§Ä¿2?"õh•œˆ?ê|¿Ìî?¼BíâØ8?©RïŠ=»?¥4ŒeÞ¿?¿˜ÐŠ¶@³?¶ÿ`µÜÍ?ç接}[(?ÇÀ,~@Ö=?¿›ÔíQ?ÂJ þùÖ×?Àä÷œ·?»µ³×´æ?ço±®×ø?°Ý+'–´ò?»É´B×÷?¨Sãö¦¥?Ä\_&#?¨;'<NÉ?çƒÀ,3b?­vŒà^á?¥£Š…r?˜T`Rƹr?̈ÈÒ[?«Ò剔æBAGN4FGL J2224.5+0353?èÃðÁYãÀEriƒQX¸À;`P‹2ΉÀ<ž>xá"@ ËÕ§½?ýÞeæä¦?Ð#$< DY?Á>ڛÂhÆ?ó&eYöì[@'Ãfœ—%¿í²æ§ieõ¿îEÊ¿×Eø?ïÿë""i·¿æ
Yº†y+¿Ô7ü:ù{,¿â¯má"ê¶AGNbcu3FGL J2224.4+03511RXS J222426.5+035445?ïÁª›ZË?yJ"ƒÀé?3üÒ#X+?&Ý~€xˆ?}êåÚì?xôõ‹:G?ï­ì'9þÔ?'$ : ú\?U¯}ä¸Íü?`TœÆ¾û‡?Îë¹`¯#?~ö¬—N?ïœ#{t?Ÿ\e×?]Ñ9)Ršé?bÌÚ.wF9?À¸íFêË?ŽðôÊAØ?ïFúó7?w¦ýøÄB?=eL§Aé?5!o´?–ÇÚʑ^7?wK1Hû±?ïb}Â3ÒÒ?'nýŽ¶'¢?Kz
Tȳ?Bõ9Œçð?'ÔwNÀ‹?'SÅí
Æ?ï4õvþÓÊ?˜Z¥t
—G?aÚyøX[?sI'#8S?—1Óz0¶?•'^i—É?îRöÒ®Û?•ÖäÅ­?apž|Æß?`zXՑéã?©¹•‹¸z?•µH$Eªe?îF•?—º~=3w?J¦ËÀÃÏ?LÍáðüŸI?¯q§"
?—Œ"R¦Î³AGN4FGL J2225.5-1114?íº´'!ëÀJ"Ĥ	_$À:¨ÝÛ
À<OÐîš|î@ÌÁën ?÷@]Øù*ú?á°Þ1Î?â5~†mÃ@ïƒ9@ØS"¥å¿ï;Wú'ص?ïí%HzÿåŸ/ۏÞ/¿Ük®Œp¿ïÿÿ" 5•?ïæ0¡¢AGNbll3FGL J2224.6-1122PKS 2223-114?ïę´5k?|âqÃ>	?eXœI…Y?jƒPIžûr?s$yŒÖä
?u²%'ëû?ï¶]¥*O?ƒ&ñ«.e?[Fíî¢?jÔql`ôµ?~*LNÌ§?{>t݈?ípñÈëÒÞ?¡es4E¥þ? ]ªûͳ€?•¸A'ýþ?¨"8s½P©?™és^Œ÷L?ïIL?Í?€*X=K?Zjë™18?PÞ/,á²ÿ?•/Éh¶š(?ؖTvÂ?ïwÉSÃu?"HµÙô± ?€Á}#bl?†\toõx–?L-ïi<T?Y®ZˆK?ïú&w8?¤c[Äí?uÃ_9_?'J9ùº°Y?–Ïãc¯UW?›ÔòœPi`?ì"Úv>ÜÆ?¦R*@²>? Dö*vQ?—õ6Ñ·èñ?³6±:´¬§?¢"
8W?î­v°¥>?"5x¡–,?X
!ÞÎ_P?^^âbV©?¤o7…Ó>+?",<åZ|AGN4FGL J2225.6+2120?®ÀÓaÿ^À>ó^1
¿À:\‰mÒkÀ<.2$?zi@Œ9j.òÝ@4ä†&ö?ŝZ³Ê?ÑöJ>ès@"éèwM@	¸§áÛÒ¤¿Õê£	"¾¿ç˜¨"HK¿é¾Ðà­ªH¿îš¿^z4¿ïò$_°¿¦?ïw:ÿ°NèAGNfsrqPKS 2223+21?ï댯6 ?d~¾T¿Ã?@I(ËÅ?AÔêÜPh‰?`aÕ'æ?aU¡ëuK?ïL­Øhf?"˜'
#?v/ÎAn?{Å3`Œ«?ÞQsSùk? þV¡f0?îöؓCX?'x?&½vF?‹y+¡)Â?ŒöǔÎ?™BI=Œ?Žm³£
O?ïŒâ5Þ?lð-‡8­?mýbœMm7?U׬ÇÅ66?…{®Ðw!+?fà]äéÏi?ïÙ׿;Œ?pŒ³YËÜ?KðÄî–?J`Ö×¾°?o,<™ÅU¹?nxèz¤u9?íeØ+G"÷?¶°'š×
?'ß²Ûô'Õ?¡n!/uo‹?°Qï7»?°¨üS{'?îN{Å	µ?›«åPÆ$?'9Äåª@¿?%Ë÷ž?¦‰ÕºÜ?™Lî-5;?îa4š*Qý?ˆÕXj7?Š~ÄÂljš?z"Wí[?£M*,?Šƒ/*‡_AGN4FGL J2225.7-0457¿çu!ÓörõÀHjœýÒ(VÀ9θ_WÀ<
¥T¸¾ù@š"ÀC§u@úÑÂÕÓ?«Fg~¥ˆ¡?´QVßµ²ª@—9~¦Ï@¦Mhky¿ÃöXak¿áâÈa®Û¿æÜrÒ¨"¿äØ`^'i¿êTCƒãNï¿ïÿÊñ*z'AGNfsrq3FGL J2225.8-04543C 446?ï×8CyT?¢^ðXR?J,èBð7?zÜÒ?qA^ò
=?ž9S*@è ?ïãŽMhÇ?sÊQnCìÊ?;$Pûfÿ'?Q®bnT/y?i
(e"~&?p(	CSœ?ï­ì¨Ænu?v¾U|ã›?\,¡[øSÚ?as­x}ýø?€ÿA¨¼®9?uU_󥒘?ïóËm"?:°ü©ô>=?0勤ÍnD?$±êjî›?T/ž+¬?89û"9?ïÖ}¯y?lU.45±§?C‰¿?6WÐcÒº?rŽP>¢x?j©Ù8†%i?ï¹ïf€?ƒ28÷X?F
s=0ý?ZË6A~ÿ?€#GDw?'B•þ¼Õ?ïwmhýß-?"3AÆRðø?ic¡|d|?pŽ›"]ü?‹Ë½k ƒ…?Kw˜Ur?ïᚠÏ?[Ŏ¾–øƒ?Fî©8ñ´?8Œôá?hª5nYùh?XJî{ÒAGN4FGL J2226.5+6901c¿êÇЈ2õ@#mfŒ&À;L‰~™cÀ<FdÆ@"퉰ÃW?®ìc.è:?æÚU웟-?ïþÖ¿ê¼!@¤Œ;ã@¾i¼²"?è0Ì ?ïò솦wοØö™NðþÛ¿â?Ö¿¿É?´ß´°÷.¿ç|<[Ðá/AGNbcuNVSS J222625+690207 ?çCîÓn
?ȱR4¢–e?•´àòɌ?œšÊ¼¿H?Ðu\ÔÓg­?ȈXi"®V?䉌>ÎX#?Îܶ7<µÆ?'/àêÒ?š[¬Ô'í¬?Õó®ùR;â?Î2+Û>ïC?ë+MénO?¬þåØõ@?ŸÔw›Tö?•i|½¦O?¾ä›—íêK?©÷9»k.*?çùÁb=ü?·µë	eéÆ?hªJâi{¡?pX'½k?϶R³'O_?·Þ&ž´½`?áûê '5?ȺQNkÖ?°2ëܑλ?«¢ ñ€?×ûpǛé?ÈÿƒeG#ø?Üð-úå?ÑuV¡ÕÜ?šœG1¤#?­ÑY(¯.~?á%%°áX?Шw˜gëL?è:y?êE?°j¶Å ôÝ?¤À"¯Iæ?›
Ów?Éåõ×vã¦?­«s4ÚJ?äçøÐÃ?Ĥ§»V"ò?ZqÌ Œ&?rB."Þ9?֝ú/>?Ä«å–È.MIXED4FGL J2226.6+0210¿Ø@àÏ|ï.ÀF;€Ü3rÀ;Y.yÖÀ<…¦Ž@!¸IƯc?ûÓµõó?Ì^ív:™Ú?¶&	>˜7?ì%vå@ú5ÏÅ¥'¿ìÉW,6À¿ïÿóÖ&ã?ïÿꁺ¿à>"7Z	¿à	bŸ‡oK¿»'®îÀhAGNbcu2MASS J22263636+0210373?ïÅ+ ü5+?tú?õÙùk?#2²®s;?yGˆ·¸?|ÐÚ
« ï?té;yã?QĈ°"?} µ.'ð?Nä'üÂ?Xø°«?}ã[_ÇBÏ?x²»Q‡?îCª#Õr?£UXª™¤µ?Ož˜mßÖd?A¹éhâ?¯}Jÿ8Ìÿ?£Vz
É
?ï•À9
?{m"ƒ¹^4?9f‹Ü"^Í?/Ç%ŽÀ%?›çù¡Î|?{=~Íðù?÷™v?‹X²×TÑn?1y	Mt0Û?$õšïÒ½?ŒDyÔÉê?‹Hþ0<Ì?ïYF%åS?"‡¶ÔN1¢?YÛMŠI´ó?pþQ}kÔ?"9†l<Õy?'›ÄYEG†?íýA?¡WúƒbwN?QÙ¢ÕÎÅH?FYr·´G?¯Ÿ³úmïÈ?¡^ìj9N?í"Q;Ô9?™ë	æÃ÷?Hª"ïzÜ?JzOŸ™<?³®!ÆQÈ?™Î–ˆ6(AGN4FGL J2226.8+0051¿ï®£Y5ü;ÀF°CécÜÀ:2lÙG."À;á/Ø4ßÜ@§¶¶@F€d?ÃßÉi@
‡?Îz°m¸@Œ:䜸@×æ\ÀË7?ïÈzW´ò»¿ÀÐâC5à¿éaJÓbé¿ç޻♽¬¿ïÿŸR@>´?ê1þ –
AGNfsrqPKS B2224+006?îÌ–{à?š@Šbp>?†Sûóþ?‡½£ðý²?›R¨zÄ(?""ÅR›ì?îȖdZól?¢€IIF±D?‡úôŽ˜ð¸?"s$S¶$Y?šï¹)å~5?—q‹J°Ú&?퓛2 ç?›˜úRæ?"ÛÔñl;?‹
ú+ºô?¬¼ÞìT¿"?–dß¾–ÿ?í`m÷\öÚ?Ý)ìù?Âšã"ü?p´Vmѽî?±D=E¿R?ñ¾Ò
?í@3µ F˜?¯C¸H}¿–? ´Gj®¼Å?¢KWSd[=?«H}>¼u´?¤:*("ì?ìþð…†»?¶ÿ
£Âío?œRHãxÔ¶?¦ÒÏd9?°óéšñ"þ?¯p
Ö§ÿÔ?êT<®9ÂL?ªvPCƒEA?ªüÔÍ-b?šDu4fbU?¿ß°)S
"?¤×199Ûº?çÁïêgñ?ª œw'^
?¨¬Èb"Q?'½ÕԁxÆ?Êöتâ¨g?¨\·Ù#1AGN4FGL J2227.9-3031?çˆv‡ÅÀMAð€0<À;n4˹§VÀ<ØYí²¢@ ò0´}Ì?ÿlº=~?ÊYÐ@tº<?i6+»W?¡±‹OÈâ@®©ÌĿ¯ÂÐË?èéÅ+Û¿¿Ö@£[å.¿èºÿƒ¿ÄõÊ\…!¿ÚÄ^Ô¡­dAGNrdg1FGL J2227.7-3036PKS 2225-308?ïÝf"X?cé5:Uۏ?1çáuÁØÏ?&¼-=šÅ?pTÎÛ½"?c+ð,o[?ïè—'=J}?jõ¶ší?0íÅLxüå?;°¢"<]a?eK >«¸³?gðFAâ\Y?ïHx`äÇ?€}Üõª?_Ð<šš]?[k~¿§?"ÿM'¦D?×]]øt?ïåiõ£@ó?Jì.=^ô?"pw©«+?ÄgÊw'à?io$kÿá?Jº†ws—?ï¾Ð~÷Ə?sÇ+§"wU?C‡ãÞU‰ƒ?9œt*T0C?~&Ä!›óÉ?s'¡tm?ïºÕò÷j?"¬Sd\õ?DÞ¬Tìã©?Wdt"VŒ?ù0ØåßÃ?'ýÈÞ5j?î²'D'!?VÌöñÂ?eÌÊ8¹«?b/àmhŽ4?£€ËIB}Ï?é™µhð?ï¸0>?j2/ó¥¹?1…p`ì^?*Äô]Ð?pMáXvÄ?j%ê)dâ]AGN4FGL J2227.9+0036¿ï©±ŸtÏáÀFÞùü°À'À9®GE8ï5À;Í´ÚgÀ@B89,qx?ÿNlªMF?¶
ï×¾ÃJ?ÀB}þÞlÝ@	†)vò@&ם`Mž?ï–<¢¤@¿Û¥oÛÛ£¿Ù²¬…Y›¨¿ÙÕyäÈl¿çr4/²u3¿Ýí¾Ÿb†]AGNbll3FGL J2227.8+0040PMN J2227+0037?ïÛL|Ž?dRå[2?PfN[2KÇ?GôÙÑq€q?l³Êul,;?`©ðüB`l?ï ó;\³›?šdò=·«?{kóÒç@?Š'ÉûL¡?•›™†ËÍ?'¯Õh[?ïnÿKÇv??îDN3?h{¬YöҖ?jïÖØåm?Ž!AíUñ^?xÙ«—È?ëe2´³&?'\æe@e?ŒQ

éÛ?jƒ"AšëX?¿ù,Hª¶?Å×ÿʔÓ?cþW3?}Ñtÿ!?lMÊ«
ãd?h'7d@'€?€üôHðì]?v´‡"«´?íí@{"é˜?¯-´}§t?å•ÐÊ"ò?ŸEÖ/l?©²'Ü2'Ç?¥Ù©Ñ‹}–?îÔcÆ°?"<§µ—û*?w´öK\.?t¼ŠäRž?Ÿ†^Ûɋ?'k¡"tÖ?徍[®#?¥g͞Íÿ? ‡*Êa?†4J;`ÉÜ?ÒrdÛÄ.?¥ZؤØx8AGN4FGL J2228.0-4155?¶üÿÿÛìÀL¤ÿiKÀ;Óúú݁PÀ<ö[ªJÁÅ@!ø-ƒpã?ü'/"R	¸?Ð`û£$ð?´ñZuÂNï?êð¾'d@fRðÜ¿ïÝÜ>¯¾?Þ?»Ø?ïʵe§ú…¿çÒ¿?›vi¿Ës˜=£úq¿ÏKi W£ÖAGNbcuRBS 1864?ïÖü‡ê3?i€M(åïä?(_)CGpp?nxâ?Í?s¾Â¢P?i&"¨pQð?ïÝá"«aÔ?r~Yل{?<òõáÍl?L£È·ƒÑ?n€~–G?oÖà¡ë͙?ï£2R@G?‹".ƒr§?^CÔ_x˜?bŒâ¨^‰õ?šç\sˆØ?‹InkÀê?ï±îjyÍ?h~…SRî¨?2îpä?)ÔýXœµF?'ìò9S?h|N¶I8?ﯟñˆª?tèfe$?9*&ë;[?,ý¶ºÛ,Ø?ƒr†ØfPô?t'Ј^ë?ï¢ð`Xbö?‡;"¦{Ú`?Mˆ‹°fQ?b­ˆdÿ?…kf¼ˆÃ?"t7'˾Y?î¢Ç¸eF?øH"?f;©+ar?mvÀіá?¤oÉéýæô?ôîI·= ?ï2gͳkl?‰4eÝ&¯?>"2)öÊl?B,l¹hS?™8µ…Ùv?‰}gjAGN4FGL J2228.5+2211¿íMÍÈl¸2À=ÊøzЀ¶À:v×ÁóT÷À<Q¬Ô	1@ë9¸2‹î@A©¸ËŽ?ƪ×Y˜¢¤?Ãõµ¹µÃÇ?ûPÔ´!Û?ü«H%2¿p?ïô›?¥¿Ô6«ÃgÉ=¿ÛRDËáë¿éâd®ÖAÁ¿ä‹*5]¯Þ¿ðAGNbcu87GB 222614.9+215540?î­¤¦Æ†j?–úómùÂI?p–¥ÉRÄÉ?j}½'¹¯ó?£àÛ·A?•e‰Qɬ?îÚ_­˜1Ã?–"Í|ËÆ?ƒ]8=©ÆÈ?….6G…gÃ?›n.$ä8?g"s—§Q?î²a!êÎ?Þ‡"œJG?ƒ%×4Ī­?')å'¾	? xù;r?ŒìC8¬?ì-`©k§L?'º>bÕ?&³.á?~Ь!ÓÜ®?·KMÔÒì?m"³­C?íµ_àæ4R?¢Ù(pyŸ/?ƒ¾I,ëÛ?zvOHWԞ?¯éÒaÏ7g?¡xàlŠïg?ìB©&ÅV?·à¨¹×ƒˆ?©0þ_ï?¤3¤ÿö':?¶€jÄL–?³SÀ´=V?í{¼µ(?ž|«Ä‹Ø?"½#'(HO?_
>¬¿å?­ñ,ÇlY?–'b€5?æÆ,'ÜØ?¥,ÙQs-?®>¿Nû?•ð
Xb["?ÍWËû¸êå?£Ü¬°ûõAGN4FGL J2228.6-1636?äå–È·qúÀK±#öM¾À:m›¨g'¶À<xÐÜüŹ@¿Î´-™–@?'yꧩ?¾âÊ: bK?™l#"¯¤ô?ܶe§"ê@²¯ï;¿ë¬k˜ÕN|?³'«hÎös¿Û†Iû̔™¿áðk֙տãȓíˆ.7¿ÚÖ Ř%AGNbll3FGL J2228.5-16362MASS J22283018-1636432?ïùY×ü?5îbÂ"?óyƒÍ–?£ €ü%‹?G¥…ù0~?4	9 ‹ÀË?ïð7È:¹1?cFn²»Ù?$íùQÍ?41hR݁?]
²?·¶Ê?ad½8—
?ïǼ†ûԚ?fÛq ï3?Q4´Ðm?[£÷0mš?wÔ¸‰â×ý?`%ï¬÷?ïêR'ôå?A^6ˆÜF•?)Pˆkƒ?
\
o«»?dX¬³àì?@ß´¾ûü?ïó–ÕfpÅ?GЋ br?.f®¢‰Kº? mZ;TÓ¹?Uuè;?EŽâiÿK)?ïÐV¿»~?}™ÔA~,-?4·™ë¯w?G·"t'5ê?v©cEn?{áä@4
?ï©$þçý?r"ÓÍó—€?W¡K"Ú»?^JX›ÌÌ?'Ø'‹&¹y?p
¼{Ù°¯?ïÌ̅ekP?_O+Ô§'?:]Ø	âûÂ?(Nzì@>¹?wóßÆY­$?^(gúþtùAGN4FGL J2229.1+2254¿ïPdô÷8[À=M5e<š»À;€€ÃàÀ<ž£;M@ ôáÊà¹i?ýá©»Þh?Ép£×
=q?¢%¹øߥB?Ø:€›k?ö¢<þ?ïü±a6{½¿ã9 Š¤‰¿è»ÞÓ_Ž¿Ð"L€a9V¿áÙ|"MÀ¿Å\Ùê¦ÒAGNbll3FGL J2229.1+2255NVSS J222913+225511?ïnv‡­?—¥úàbT)?r–^¢‰ïŽ?–;Aß_å?‹/3X,é?ƒÇ¾Ÿ%]Q?ïYÝÔ±óƒ?íܯu¢?nÐ^fºŒ•?s`ÞXb²?ê9š*Ž?ˆŸKó#0?î¶Òíx=ÿ?—ÍáÏÝ0D?h†r³ñE'?mü³Õ
Ö?£
iúëO6?—"¸Wj!?í¥'‰:Yv?Œ<!?~ªêX‡®E?b4gϓÄÍ?°é=áì°?‹åÚhœC?ïD	:ð?ŸÖ¾›º8Ô?i}ºñþ˜?œ¤WÙÛ©?"MƼ¥RÙ?Œs-¢1m?î"ŒðÎ?©²£…ž¦?|ÊÇ=މ?'öýÁÂ?ª\ÚՖM?§â¤úp«?íûþFӊ<?æ'ú%æé?n»<Dg'­?j¿ŠW%?®TgÎTé?F,¸"f8?èµIÈöÔ]?¨""‰$Üw?"•¹x!ÈÔ?'Ù‰[¤d¥?ʸ!­Wo0?©HÐÜÚjAGN4FGL J2229.2-6911?ÞÖ[8WVËÀE	 :2+À:–(òÀ<~•rÃkû@ÊIÞEp"@_þmXÉ?¼L^}cØí¿©"¯#æÜe?ì!$þ<0ˆ@æ)ë
û\¿á¸Dêë›Å¿ãB;䳿æ§Êêt}€¿å'Paí/ï¿ê÷¢cl·¿ïÿ¦¶tFAGNbcuPKS 2225-694?ïÔ%ËZu±?jsBáËï?Tá÷ c?Eðb¦ž?U?p´×ß÷M?h$h@Ž?ï¿ãI³I»?v#©ƒ£u?Jé°nˆ•?RÑ¾Þ~y?|±%
Âì'?s™Œõ™&?ïd‰ê‰–?*œn‡³m?k7ÏDäE?k•ßß«¤?ÈÙõ•ž?|q^Tݝ?ï·2X/«?\rcûÍY?a"jyu«¶?CÀ"P·\›?{՞c ì?Yó­[¶"?ïh¦,Od?ˆ ¼-?s¶Bæê?h†RP@ˆ?Œ®Ùc¥?"ÍÎ&)?ï1W.¡9\?•Y¿Ð?<?aånE¹5×?kŒE)Ÿ?—˜l\škÄ?"æ"L'O¯?îגp…y&?ŽÁ&ó¬,?wa¢¢ åŸ?t7"(ÙS?Ÿ5IDñÖ?‹Ë'¢úøL?ï(Í?I¨&?}ÒàûÁv"?z¾È&ô?f¤?"Bt(L΅?z}腇`SAGN4FGL J2229.7-0832?ÐB/*÷
ÊÀIÚÃ.¾YÀ7㸫­˜TÀ;¸<ù…'@6r$àŠ@ÉWòÓÈ?•ŽšPèj?¹^¸`óϊ@þU@ÓfI`I¿ËU+«u+¿äœ.܌¿è]º|h0¿è½¶ÿÛíÒ¿ìÀ©s+pÇ¿ëêM`ÛâêAGNFSRQ3FGL J2229.7-0833PKS 2227-08?ïå}ü7Ò?]Ö½¶4R?VrxÆ?UŽ¼Âæ×?^ý•SÑÐ?Q$v(é"Â?ﶰ™õ#?ˆÏôÔ»Ÿ!?W=Å&¯?ryËò'v?~؅ô;r½?ƒÝÿÂõàÑ?ïlÄRČÑ?'Z¸.ñ_G?«'Âò?Š5CÒ¿_d?ƒ#Ü¿cK¸?…"fbà?ïó]þô›?@Y)±¢´?A7áþŸûä?/ÕQFû?P©ôãpÃ?7^Ä0Šg‹?ïД¾¤§%?lQéþËp?Y"P³7'?U«¬Ýj@?qpûžþÿ–?f¦ÕWæ?ï_{°Ðlê?—¨ø:?k*Xi³­Ù?ƒYòèOí!?«>ÚÄö?"bÁ+´Ý?ï4¼'°?"×fómå%?ƒ¸ðëpÂ?ŠùÖ_—ý?ê¡VÎÚ?Œfß뵶?ïâ3Ϙâ˜?^&s:îì?Upe؞Õ?Ll{'Ÿúi?cDøsèŸ?Tº]ë_ãTAGN4FGL J2230.9-7815¿î®×"ûÀB="V!uÀ9ü›A9†4À<NB€Æ@$y&5@*t:dÜ?¸LêijÓ? §½sñó?ääýp-º@
›™pÿÇv?Ú¾..½¿ã²xÞ8/¿âhrzpßf¿åã¡$¨Uõ¿àyâš'¿ïÿ¶cÔ»¯AGNbcu3FGL J2230.5-7817PKS 2225-785?ï¢ Ã?Pqï=³gh?3âŸGZ"?"'͵é#?^9@'^Bq?N£èMÝK?ïØòÂù1?oƒ ½áÄ?7Ô½lÉh?Aä3Vïj?rŒº$1ð?mC@xÁ^ç?ï°ÃÒºf?tjqýå×?Y4ÖPas?_n´[ñQ>?€¨‹ÇðTF?r|!¯?W¶?ï½ìc"Îu?Z⊩Zºˆ?M ÊgœY?0™¿†çùZ?}f<G~!?Yá¯Ç·D?ïÙ2ÆѶ?fÈljì?I‹²ó5?<Í/÷l‰‹?p5&)?d(ß8ßkr?ï…30g?ˆ,&¾I–?IãRÉ·™ ?TÖ©‡Ñ?½ë?‡6Lzÿf?ïhÀÞ¬ô?…ZQ(h^K?iÄ%ÊL?o3`þ¾#¡?‰LjZ?ƒC¬Â19?ïHhwkO?y%ðÍ+›%?dxcC:J%?Q8óΰ²ÿ?"cä£OD?wÂS+áPAGN4FGL J2231.0-4416?íîÞr;±²ÀL5'Ì÷À9ÓÖxG9zÀ<†óEšN@tu%Çe@8TÛ#§¥?±vp_8Ÿ¯?¨œêB9Lj?ðxë¤(hÕ@,(¡3ìÂ?ªÛk¡
×.¿â}5´Âë¿ç "¦£m¿æðÀ'+ç¿ä$?	ˆ?¿áüâ©­ãÓAGNfsrq3FGL J2230.6-4419PKS 2227-445?ïû:õta?3ð''¿7?Æå]™Øl?,Mè‡L?A67Ó®®?2­Â³)¾?ïòæVáŽ%?aªJ %?"ɂ¨‹¶Ÿ?6¾:µž?WÚ"$?^Žm,†P?ï·±_çyÕ?ušçèÖ‡?R®-Šßºä?>íWó^Y?{ğì>ä?u9NÄHð»?ïý"ñœÃx?.g?‡%€éõ6>ñ›¾'O?0‡g»`?tMÃÜBú?ïôjÉޗ?JÅrq˜?!L+W'»?Ö8®è3?Uæt³š?JXúû¯?ï×ãáç;8?y‡³ØÕÆ?3>p•
¬?FŽKΜë?rÚ-Ñ©Y?xm#ïq[?7BÀ?z§€ ǂ?_Š˜!Wê&?Sã÷óÙat?‰f¨wû0°?x–ÿeò<d?ïù¬0l{Ì?95ç›tŠÕ?ÉÅlº˜W?swL®¦?EvíÍÏn?7.¿SÖoëAGN4FGL J2232.3+6246?âa«'¾¯@G"#ρÀ9¥s¶±•À;M`ÈW@b$uÖÿ@Q*Dw(V?ËE$wX§?ÅÍ£À#@w]š
_?ü…ktm:@?ïÿôa¼2¡¿ÚlUÿø¿è#†b/J¿åha}ÉY{¿ïüG¿e ?ï'[>ê÷ZAGNbcu8C 2230+625?ãÏ|¬Û?ÄM¨)UK?"É?¾J¶?~]œyܤ?׺¼©éóÏ?ÄD'&ï¿&?à&çc.¬?Æo#ÖÁ?¶i–~
?±ïÖ7?Ú˚-?ÄQi›?ãª,ÉYH?±Â쿪|?¨ƒ×9³"?"3¤äØ{?՛+…ûé+?±6Í'?Óã?ájø5J)?«Öïª(?¼oT¡—êÃ?—Äîh…?Ö½Tç/pþ?§€ÞÌ·P?؅´úñ?ÄÊNü'a?'¯‰u(-î?‰ŽPfÿü@?ã/©7¾ª˜?Å:ûËà5?ËwƋE²?ÃIãT^ã!?Ä2'aÊ}ñ?ÁÏN˜ø?äiÄÈO?Ç	ÀÀql ?×+Àm?²;ïûh%4?³éàö"Ò*?œþùv¢>q?áø®…'$?²¹m±t±Í?Ë(¨;" È?¦áÄ´-!T?ÈC7o?­™Qö–?ã%#[Wr?®8¼vGÂÓMIXED4FGL J2232.6+1143¿ÜôBL¬µÀCJ¤ÁëÈ;À5pP‡×ÐÀ:{ô°@¥@ÖÁmH-@–™â"µ.?yW§lý¤?µ^¢¢¬½¹@9–x?'æ@&sg»Ðü¿Ë˸e6»~¿àf·#îÒ¿ä¿ëþ@bF¿äGÊß·¶¿é®‰`‹é¿ì¢úkkˆåAGNFSRQ3FGL J2232.5+1143CTA 102?î¿Q£ze?¦ÆªðjG?"žÊ.W™?žf7vÔ
?•@ˆA"¯?˜ßtä\Û?é]öP‡_Ž?Ó4¼Rß©?À›`Ðò˜±?ÏÓ1üã?³Ù‹Öp64?Â$>ÉÐ?ꦈ3&[?²­'âd?ªçuЩµ¢?¢BÂç(•6?½X{yaÚ?°qXa.ÝÓ?ì>ó"ol?¹–7!?«à.ž5ü	?¶¹LºFL?°Pӓ?³û\úçCD?í´[RrNã?°ፑ2?T«¶í°?"eø©à¾»?¬õO#³÷?¬D·­t?äâ':ïY?הÉÝô?Ïî»:Y5?Õùœs¾"¤?¹"÷¿øP?Äd2@?ëNvÈ*Èù?³)ȾYÉH?£\u¹ÏöÌ? µqh,w?»ÞàåÕÕ?°–d3´×?æ–ÞѺ¦?̽	~al?¶¼~q±.r?¼.Y?óq8?ÊI]Kà~0?Æz¡;¤pãAGN4FGL J2232.6-2023?î;50l ÀLÓ²VÿÁÀ:ä#åGîÀ<›OÚ2æÝ@ 2ÀD©'V@ÒÁ&¦]?ºz#À8•¿³"F|s)?ù/JUŽ§Î@P@à'¿ÂËr"¬Í~¿è¨nÿ<5»¿ç¤Z¬1¿ÇͼŸ9¿ÜÔWZ¯Îå¿ÛLyÊÇ9AGNbll3FGL J2232.9-2021NVSS J223248-202226?ïè1€V™?Y`²
—"?5£–•¡?$Jh.äÑh?e
PC?X «i'?ïÛJѵiÚ?pÉ7ó]™‡?>BR(Å«?IÐll9?pzRö¬Î	?m{0HÚPÏ?ï&FCcá?~Øژ?UÆç~?;^ "‡b?Œý'‹2?}ܴͯÒ<?w¸÷`}?au
!xÁú?C59+3ê"?.¥ÿ=|ç´?~Í|hè?a#àfPü¦?ïÓØ.L;?j™²bÐ1?E²¸­ÏKá?7é2÷ç?s]'åGþS?hÌòÔù¸?ï˜H²\šF?‰=vO‰ø^?M—<·šâß?W³ºC; ¶?ˆ_'¿ÿ?‡µÍ¸Í>÷?ï]ÓG?‡&v-Ñÿ?_‹ÐÞ9?N¢D'i?›{ÿs?†ÓxöQyœ?ïi"}±î?'ÿeА8?a…Ù¿=³æ?VhˆX`Œ?š\"Ç?'ž²öËmŽAGN4FGL J2232.8+1334¿ì:ðcLMÀB›3ÁÎl	À;{]š
_À<»£IEÄ/@!§â^¯bÚ?ú¯4^¬^?иn¼ W8?¾õCŽu#C?îõ'àh@žwNëö^¿ïþ!¾–©$¿ïEHßlâ?ïÿùëñ¿ÍAÒ2g[Y¿àÔ£éտ̇é­WAGNbllRX J2233.0+1335?ïß­¾Ù]ï?oÆ÷<¹L?&-† Üßþ?mBæb¸?nïhºÊÝÝ?o+2ÆïC?ï¯Ú3ù½Ø?}¹TMÖ?R´9jA?]Zás0!þ?²ïÈy§É?}ŒÅmÙ\ˆ?ï" i f?Œ2€ª¦?SýON¯T?<¨â>åÙ?š|䕶ù?Œ ¤±)ø?ï6¾²ÐÔ?vÝé,çX+?;וd–?+ü;^\Û?˜¼¢ób?vÈãYRø?ïΎuú?~³`D??5)ž¯îÐw?.!\rÉ­?w^ö
®?~tl™Z?ï+‡Ñ"Ðm?›ý,ô§G²?Z†˜}•M?kÕ†Eà"?˜æœLit•?šñóâ`=ö?îµÍ`Ô?Ø!¼(¿Ü?X큼šÝâ?L'¶JÚï'?£Û›r?»E|;-á?íÞoêý ?–D‹Ó»Üî?H¯üÊäw?F³îj«Ü·?°ÜuHÚÎé?–.ü¬^N\AGN4FGL J2233.9-1229?
!ÂÀKV®Bž
BÀ;"k"ÌÐÿÀ<™êBÿY@=^ú·@É?þyòoÀ?Õ<ÿD™7?ÌÈm×ôÉ?ôré+¨$?ý°|Ҏ'º¿ïᕱ­Œ–?ïöUç¡9¿Û(øýWY-¿Ü!YÁèBI¿ì‡Ø¦õ¢¯¿ïÒ@tdUëAGNbcu3FGL J2233.5-1235PKS 2231-127?ï£*dW˜m?y¯¨ŠßRÈ?`Ûi±–.?R÷¬š3dµ?ƒ0ðÃå?vû"1
 ?ï¨uÐ;?·ž"±©­?_Uß^™¹?diψ..\?øsŒ?};g#k?îÙ͠ԘÀ?'Âiª:<?ü….£
—?'"åc|?›È	Q_¡?ŽIÔ¯=r?íqÝé?}g5$lIi?'wTÒr²?gÀ–uN¤?¡fœ)1uÆ?y[•(^Ú?ï[Píbf?‰"êÛ·"ƒ?n$MBX?dçoO?ÑoÜ¢Pú?†à[nŠÕ?ïì,IÆ.?šÅ³£"À?qמxUÆ?Ni~=…?™'×ÕáÁ?•ol~ÁA¢?îh­ñóÖZ?—ÌÞ
¾ŽÙ?†'W'ón2?…éø§}$F?£ÐÊýýŒ×?"ñS~}›?íKÐË+"`?"ì"·ÇB?‰G>z[ˆ3?}«ÁwI±§?²x'×Xký?"	͕;êQAGN4FGL J2234.1-2656?ïšK:õ†ÀMî£À9F®×ï?¾À;ãð/¨d8@>|ÔçÎ[?ÿF7õÿÌ?¬¹¤?ԛ?²Râ¥üÿE@4†º™Äb@[ùëñ¿Ö9Tç¸á¿Í6ºý–š¿áÃ^6=¿à÷ÍAìa¿à¿ÓÀí¿åÚI{«AGNbll3FGL J2234.1-2655PMN J2234-2656?ïú <Æ?Ad+A¯õ<?ëóßÁóÇ?
Ÿi÷rá?C!4t??±õ¶ýÁ¸?ïñþvy??b(-Ï{½¸?%ín pæN?7@†;Ø(?Z"TÏtKÉ?`H"˜!?ï¨w©ý?~SbIÁ€?h¡ÓV$ƒ?w³Mèž? »0?pï3ZUÐ?ïôþróMÑ?8rrW1—Ò?
ŸàUÇÅ>õ¸áî?U.üÏÙ¦?7íu¶ ¢?ïöy…
V¼?F†Õ;³‡2?!jýñFoÄ?$'iÎdd?PߕÙ?D‰&œ?ïØ:Ï3ÚM?y"xà½v?;\R¢‡	?QÓ¹AR?r1ҙé?wE>+<w]?ïu¾imèø?…ïªÿ9ßß?s'LJsëJ?€vê¾?ˆÏâ+¤a?}¼‡ç?ïé~³±•0?RdåëÖJ?]h2š—?áô ã2?e®a
\©g?Q¼E­¨?AGN4FGL J2235.1-0623¿íô;‹=Ø ÀIʱþë-
À:ßó£Ñ+À<"ÇÝyÃ:@ãܚJC›?ðà"¾ŽE©?Ûy—¹>Ð?ïm8bGõ@æl£—I]@ä(Þñ¿à¥TþŠ	.¿Óiû±¼¦¿ÚÿÔač¿Ú®b¾ç	¿ð?ïÿÿÊPËAGNbcuPMN J2235-0623?ï——zŸG?©µùx[Ä<?qTµÒæÂ?†ÙIª:s?˜7ߗ	.m?¨SW
T'¯?ïuÃØv=
?'M™–¡‡?màa7Æ÷?y''…=?‹ŠzÁ?ŠŒ>î\§?ìaT4ÏY^?¥þ÷ïʯ?«ð†'"?ž­˜),A?®æÌ):$?¡ØóÉ&T?îÙ
"JB?D¼ÃKa?ZYÓzJÒÂ?Qv¬¡â}?¡œˆÎÚÇ?ÜŠÚäèw?ï
Ps_ô?¥f"ü\Æû?w1Ïʜà?
;¡Ðw?˜é}š{?¤|Vn'ú?îpï?N°£?±øo˜V?ŠÛ­ÎQ?©oë!+Ù?¢: –±.w?¢h¿Ÿý0Ï?ëŐZšo?©}	lŎ?¨Ž·-ø7"?ïêÔ··?µ'ç
÷¼?¤ÿy·îh?í‰îµÔ?¦(]7Û¼é?`€{1Aõý?f‹˜®ÇÝ?³3|³°¬?¦#ÕÿuhAGN4FGL J2235.3+1818?µu¸.À@ìƼèS;À:i"6ÆÀ<h·'"…@ğ+ÔÅ?ÿƒ†Üþ?Ï¡Ñv¹?ЙäB4Wö@RóݲÎ@:äßJ¿Þ®ïÔ;V?ўY<1^¿ãÜÝ¡0fпÔ<_p#¿ìaÈ"n·¿ïÁmž%øAGNbll2MASS J22352860+1816356?ï—ã˜ãˆ?:YF!?cHµÛ¬?U]^ûñý?…4ìXɾÒ?~ƪ,d'?ï¬H€Lk"?€ÂËg­i?[âeê Å?dùmJqÜ?q"K7ë?z9H˜Ä‹K?îñ¶qt? ?'·v¦ó?ƒ†Š
")?…j_~DŽ"?˜ìĈ?ŒÀ'ÊFËñ?ï¬&
õ?oªÇ—d"?{œ¶Øbbç?ZeçÒ¤¸?–#Ms6"£?j/Vž4?îëáäGN?'ú%"LÒ?~Cñ÷ªƒ?tZ¥Yíl?šòÆñ"û?Š£ØBéã?îãøÙ¬?u?››ZV;5?p¾c–êõý?yLÈх?ŸQKè"åã?—÷åúý)?íÙÍѯŠ? ‡ÿñÅÞ$?•	­¶ƒ Ž?'lâ]V?§ÞL
5!ê?˜\ŗ"?î+V{ö?‡9["‹¼?ˆƒŸ_ÀÕª?s¶7ÇÝó½?¨ìbȯÙ7?"c—Õ ŽAGN4FGL J2235.3-4836?Ün;-8ÙÀL
×6&-À97½8SLÀ<YÑ쒛@¬Ê"ùT?@o`àëh?¤Ý,ÁT¹?–ä&¹/ê‡?æãôÑΔM@Ÿá∠οÝR°[Ò䔿âÇZ!‰'¿èý'¬¿å"]àZô¿æ4²G^¿áHrÏCAGNfsrq3FGL J2235.3-4835PKS 2232-488?ïöf"vû=?tÞ)1a(?#lqBPã†?LЌ9ŽB'?PÅhnš7²?qW&‡E/'?ï廊ñM?dgo2ºRÒ?*`"¦˜Ö?;"MŸu¬?]rÄ7cÙÃ?aì{¸H?ï±6?ynŸæ$å¥?Tñ&Àñ?\#h
8'º?0±\.®,?w®¶€{Ú?ïüYíöØ?#†@ù?²*/Ü»G?1âèq_?7ð¦æÑêý? d‰Ü²Üµ?ïò²	Š‡?bÑûøæ?#o3}6B^?%IJÛ¦ø?X-ä¨kù?`ù¾Ìз?ïкۼ1}?iž©tÀ3?6ÿ˓úÒ?HtXÿÁº©?v2•g|"??~*[zÒg—?ïiY¡ö¤%?‡'Ÿõà3µ?[ë€\Ý?WJBaV¯?'¿Yڂ?‡^âÅyʱ?ïö^êNÆj?Cu^E—y-?4|cd­å?)s.lð.T?LF%¸	ъ?>÷sÿvN{AGN4FGL J2235.8-3627?ïñ"G€zÂÀMórq6¤À9}'OH<°À<\²ò03¤@§Íęw‹@Qæ­j1?®Ø\fÍ?³©/¶@ð{xFb»@
C+ò!?ÝC›=]¯¿áÜ®ÙÄ­¿ãOx¶Ë¿ã	U~·–¿æ`ai§d¿ïýüðüAGNbll3FGL J2236.0-3629NVSS J223554-362901?ïõĔçO§?Fo'­¥?"~§Ñêù?Z)ŒÀ°<?R'×4¿ƒ?CîÖ¼ݹ?ïâÛKZ?p'Ìtl¡?>qn§…è?K*òm£›@?iVÇ_"?kÛ2\pÞ­?ï¸2#Ç8?tÒè¹H%Ö?ZÖ\&tC?g\®Ÿï­Ð?}1W˜Ø;?q}å¿P"-?ïÔVJ(\?Q"×"åªä?YV•A©ñ;?> Ñ°åÙ÷?oN_N¼?K†,¡tÝ?ïåÔìUÿ?aîʲ›<?8L¼"E?.ÝKNmþ"?gô«%™ªÔ?`òê?Óù?ï²Ãæ³m?†`ÚVeª?OQϯ͹Â?^.bI¼X¬?Z!ÓÊÿ?"T·àRè?ï‰ínzS{?IºÃ9Âñ?d4µVs/?l,¿‰ið?ˆww
'?}XÏ«­?ïœã2"Òµ?o•Ÿq?lÈoяKW?W…¬—?•`)×?hGbþœƒAGN4FGL J2236.2-1706?íûµ³çµÀLŸºˆ&ªÀ:'Û ¥&–À<k—€º¥ƒ@øےbm³@›ß>¿Xp?¸2Ó	'¦?¹•b?äض%ö@<ŽP».?ìÎø@n?¿Õe;Ãûm¿ãÝK8)'¿äúm^Ó!¿Û9æ@;Yr¿ç—ͤ?»AGNbll3FGL J2236.0-1706PKS 2233-173?ïÇî_ÞPÈ?n—Á¬K
µ?IΩyÁ!?9†Ó1\?xÎúú´ö?m#1€?ïÔÃ[*7?qÅeIÂ?B"ýMK¡å?G"`¨ÑO??sZ®˜Æ>?oÒrYü)?ï51€«Œ?‰m›´l?nžzÿ
ð?k¯¾@Š?•Š
|ÓÅ?†ÔbÔû?ï—û½â4y?cO/ÐÔw?c-IÄ* ?HuF_'?…5¾'î["?awä1Õ$‰?ï|;[1S?œ¿×,Šj?aµ/ù&"?Tß¡Dl™A?ŒƒÝFvï¼?€ãT«*t?Ùqg?ŒLEð?U
AEsŸ?aã«	?‹¶axqß?‰äfÀ€¥?îÀÄ£*	?'B—؍ðû?~P#–¹?vdœà쁂?£1	¡	<¤?Á§ê:'?îùqM«Š?~ºER›áy?x!/ƒ-úî?eN­ÿÙqÒ?šÉŠ'b`ì?{f'Òt AGN4FGL J2236.3+2828¿á¥eeñ‡¨À9¦M;òõVÀ7Éá|‡:À;8œÿ¨@k'HíYµ@*ˆïþ*=?˜N𪢀?ºÄñŒܺ@ Ú£ßm¹A@@Gbj-p¿À¨c¶Þ£å¿àz¡†Íå¿ãwœ¹ßŠ?¿æ#… êÚ¿èqJÝõ¿äy®ý®ìèAGNfsrq3FGL J2236.3+2829B2 2234+28A?)Ÿ¦y?wb~ˆ?PnC²ߣ?MuD¢‰¿?}Úª$¾Å?tä‡À¨?ïµØ¡c´Ó?"á¿€Õ"?T–{}"
?dï/2%¡º?î%iŸ?'J—¨Óž?ï…<È]Qj?öÍôŒ|?rš\ÛÝë?ƒ'€¬Ë–?…c¾0öÄ¢?ˆô¹	}UŒ?ïʾfúØE?a9‰!õó¶?Z)•ZYºŸ?H‰¬µFM?tg@>Ö?Zn j?ïªqäÚñº?y½²E<–#?Re3Ì(?Lø5[4y?ƒš.œwÿ?wýŠ;L7?ï2v¶Ú`ù?ž¼1¹Ù?qŒÇHÂ7?'ÉL¥£$Ì?•M÷eÄÙM?œ"°¿«-?Nl…Ë?Š•ö
®¿?q$³3¸°?}g«2q¨?…ˆRÃs-?†¢F¼RS?ïìu?})_¾
K
?là"¢?^ñÀŸ\o?ˆää'K?y+¹HãØAGN4FGL J2236.4-2309?ɟìAå±(ÀM¥ÈÉ2
™À9á^"ð•)À<drr
c–@l#¸ìÆ@P%çñ?»D?JÑ-?¸ŸŸ˜O?õ2cʪ³@uåµQ¿ãSe¢òð¿âµl]÷,¿êž€‰'\¿èl7`¿]¿ïÿpŽ• ¿ë@ðàþ2 AGNbcu3FGL J2235.6-2319PMN J2236-2309?ïêúòñ?Ÿ¨q"ÄÏ?EYDurÌ?|~¼Ä¥	²?__:{
o?—âXšãÖ?ïã¤3jTv?qôüí­N?>‰'ÔF?TMî‰Vɚ?hŠ§Ä˜¶q?mŽ\»ù?ïÁO`epr?rþñ&n?V"Š+ƒ	·?R\C¯ÐB?yÏ­_C¼S?r8Š­þï?ïéL1(cn?FÉ#\N¶?M/ӁRO¾?4°öÅ~+?^ϳæÝ©C?@Æ/Ä	\—?ïðk=nS"?znÕÅ̬Ü?Cf\¿t*™?]^ÉÚïG?UvV^1"È?tÙm€÷5P?ï 7qË
I?Žt
Y_
à?VpxFŽ^?n%iÔÎ?… 5†rëó?‰Ì©Ô^ÃX?ï™zu<?~Ëõ9
?b$ÿ;{€{?m³c朙?…0¡ˆ{d$?z£5äPV?ïÁÊéÙß?iS,|åv?e±ç)؉?Vhx­šfK?t'±ÿß!M?bJ^7ã°
AGN4FGL J2236.5-1433¿çA¢h0|0ÀL›ºÜ	À7™šFgÃ^À;R; g@Úô	Q¸Y@"3ÿ
z?–A…s"?²-í_O¬ø@Ï⾦™\@çv¹iÄ¿ºþÜ>"Ë¿Ý 뽨¿âÔ"Œò¿⹁@‡Y¦¿æ€ƒ}Îaø¿èי¿"9áAGNBLL3FGL J2236.5-1432PKS 2233-148?ï䏘}©"?aÚÐ3Ê2ð?:·*"|É?4"¬²:V?h'1ÿ?`̽'Ô2"?ïÞAÕ@y?v²ŒNÒ#?@p:ᄸW?^vɾÛž?m¢A™K?s³ge‡Ë¾?ïÀSCì5j?{§ÞÙ"FU?bÈ
ºÏº?r&6iÙ@ƒ?vr]ö>ñ?utÏ¨ë5?ïõµVìÿP?>[¾4ä? <ri?
\]Ÿ:»?SkMìËŠ?=6Îc=à?ïÜdè»&?b&ÕCID?6ݯ8ÙÌ?0ÖKÃg¬§?p`"sØí?a<I#êr?ï±ít<	?Ž½ç‡}?NÚ֍Ÿº…?h±_·W$?–ë+ïx?Í0ä"+Û?ï·ªù_Ê7?½"ƒ¨ƒ§?bbZ)útÛ?ra²v,%§?zùVU:±º?|ô3«—‹?ïë»uG¼?UêµGúZo? çÆÒ§¢/?)dZH?càÈ ýeñ?U^m}ïµ~AGN4FGL J2236.6+3706?ä,8 /ŠÝÀ2c¥]:ÉÀ;A¹'ÔZ`À<šE'±H@!þ75Ì?´?ü<b¼ºh?ËóÍ–&?˜ÃOܝ`Š?ÏÃYª¹Ò@k,†›»?å!͗¿áìv0í¿âeˆðÔê¿ã<`®kŽ¿Ëßõ½‡¿Â"3£ñaWAGNbllNVSS J223626+370713?ïä HW?`ôՍB?%0ˆ#F¡?³øý¤7Ì?j \ÛfZ?`c±b³ˆ?ﰔßíÞ7?…L·†OÌ?N]¹"ùŽ	?Vē贚¶?ôì`ÆÖG?"Q—SA'2?ïMßÐúGÉ?ˆyȓ¹"$?P‡™Øì?Z¥·1tŠ?•;ŒP¹^?ˆ><sKR?ï'm¬ð}E?uI­—'9?:þcËЋÍ?&ø|ÇÍâ ?ŽŒ¡˜ÔhF?u]¶)HSü?ï½¥¥Òž?t²ðßyîF?:"¹×D,W?-_%_àŸÖ?ՁhÙ?tJF$1£?ïP؎]6£?–	•Éä?\/gë,y}?m9£ª1žá?"!÷´r‡?•-héò?î¸1s¯>
?'ÄH9—µÆ?Ukx®ÿ¾?\¼L7kE+?£Ñ¦Y?'»5CÛVe?î*9‹«´?—ŠÝ´¾'?QäßH;ŒU?Ià5"â?¬Í@I£
|?—µ5n†L^AGN4FGL J2237.0-3921?êF낫§ŸÀMË~dž<À:–VîúÀ<ˆL×I''@léú=|@–Íl.ýD?·üß¶´]?µy™ßd©ù?ûÖÃƓÎ@՜9\-¿â¨+BNC¿â«ï§Ã(¿æ~¸—·¿ãÿL±‰zh¿ð?ïÿÿ>¹úAGNfsrq3FGL J2237.1-3921NVSS J223708-392137?ïîDJÿúï?oÅ횭¬Õ?0I®á?*±'Ž¹BÀ?_o笿–¤?oS!Òn"?ïòˆuQ]7?b6_A<ä?$Üt'¼Î?6"ÊcÀ¶•?XS†²Ý‹?`|Ù
#?ﭕÑ|Ρ?}"Љº?kÞáÞhò?wugö]c¹?{E¦Aæ†à?s'€¨c)?ïý2nì™?àrö9X÷?·­˜)ô«>óÃy…«ßè?3µš`÷p?ºè–#dÖ?ïê%ێ?aÒÈ;Ñèð??"û§ÖÁa?8y*#Ö·¬?aö'–.hf?a1(~}[?ïٕSٜ?xÄèA
a¡?3žÜ	¾?IÅ "™-?qû†}@ö%?wk£à:?lô}ž?ƒIã*1®Û?pWO‰èè?x±Xî‹;?†ª¡<kú?|[ǟ»ðz?ï÷™"uðó?A
ÙCâI!? ß8K‰Å?è°lš?Mbâ9Z(??LêéڞfAGN4FGL J2239.2-5657?ÛÙÁ†?ÀJã—­À;o†§NŽÀ<ê>Ä`î@cŠ!+ž¿?þ^ã MèÁ?Ù%™A¯ø¬?ÐG¤"Y@Ž?ù–p4Eê?þï~'£2?ï²µ>»§‹?Š8=3<B¿â :<½¿á°ìœuìì¿ïêë I÷p¿îå[n»Ÿ~AGNfsrqPKS 2236-572?ï¼O@|iT?oÛÜL®?SµK9ƒì?N¾Ûºòç?|ëéËrÉ?kÒm—PrÃ?ÚâÜ{?‡«Yr}š?hw×Gew?p°t .-?‰Ah	 2?'Wuq?îÓvٔö?'YŸ©ˆb?Š£å_Ü,¾?‡°­#½‰?˜?2K¾T?‡JJǑ‰?ï8scúÑ?uÂZŒJG?|€`ρê?dŸa)ô™½?•øÙ[€£6?pϔÊéb?ïbz6ãýý?";t>þø?k?&µ,"?cº‰÷5¼0?HÔJ¾–Þ?'Xl<dq?îÈq§ü͊? à1âÞـ?vqc³ñA?*ƒx5í? ª¹	s¸?¤Àž~ e?î34Y«?˜40D|—ç?'õÄòö¥?
ñC˟?£T*=…
…?'Íû¦6?î5•†1?Ž2ÛŸ'x?€³kU¥*G?uˆë²ÿ8à?¨yÕÞôÞ?‹'ËQö¸qAGN4FGL J2239.4+5130¿énì`ª©À¾ºñ6;À:!K,F°À<N0å{@´Î3@*y]¹ïz?Ç!'al¯?Ó]‰Þe¦x@+‰>@+±ÐÈ?å+$;H«j¿Òë!Cœ¿ænÚs~|Þ¿éÑÇ"hà"¿ïÿÅ}M2¹?áEUt¦›AGNbcuLQAC 340+051?æDƒõîY:?À4[hþ¾"?"ºk¢ð˜J?†d¡¯¢×?Ò;QZÀè?¿£Q­‹'Ä?æì‰G"a?Āxõ_=?#Ó=ë?'å ֏CT?Ñ-ÏXd½f?Ã_h8.q?ëv£9D^?¦S@¥ïš?¤jrAiky?–
â°}¥Œ?½É^¶Í?¢As
äx?î±G¶"?‡\÷Þ»#?ŽLPc&?m¡'–!Ê?§.r5Ô-?ƒÓŠÀ®ë?Ûö"òÿ¢ž?ÂR*^G?ž7.­vø?«ì9|?ḁ?ªŸ'UŸ?Ü#æ¿g3–?ËT7øóNõ?Ø×+©?¨Nȳ45Â?àÿH!NP½?Êñ?Œ¡¨K?å8;üc?±‹hÕ0½p?´äã5Û3a?Ÿ±pc¬?ÐVO9p†r?®x©­Ä¦?êÈÿu
³?¢"ÙBKàñ?¡¬›€®Îû?‡$>JSæP?ÀpÛL
ìõ? r
±hMIXED4FGL J2240.3-1246?֑)"D ÀL
{é…jÀ;WÓpóˆÀ<Œå—ží–@ åp…ùÿ‹@?ßÁœ"?ÃCeÛQ¿¹µ	a¨'"?ò…Šƒ| ã@ÈæšSRã¿îéºy
2?ïœ&Üã›E¿ãŽñŸêì¿ã¶,ýx¿ßS€Èп¾`ÍöŸAGNbcu1RXS J224014.7-124736?ïc'ô0`g?™Ё—'.?M{wËrO$?Sï!Õ¢'F?'¡Å»u1f?˜³N{­T?ïÁÅ(#ñ³?xEGº®,?MþÉ«yzÉ?R—"ù}J%?{]'©Ñ¥C?ux‰£>à?îæŒÀ(ŠÊ?"pÖmÉ?`•dÁ£¶l?`¼›3‡±? Ý²Nüz?"íBâHw?ï/jHÉ"?4öø\'?_ÿ´áy]?M¤C§r*D?˜»ª¡ºá?;WdUî?î½æÒ©Òï?¦W†î~õÀ?a>Soå%i?`ü͖Wb?£
­œÂ;?¥òK6Š*¼?ïa "€GZ?"¤1Ôâ'?aE)†p?oì\Ăû?'£H\À´?'qjM/ò?îA'ÿC?›•^"AY?f¡ŒÀ·Ò?b£ërûXO?ª|·>MÌ?›xSP°"?íg\ÀÓN?žl˜Â­Z?w'Èx?p["žX«H?³ShMXM?ž¥-">AGN4FGL J2240.7-4746?ë鍁w'ÄÀL¡R}ÔAÀ;Îj[¾mÀ<Íëýê|
@ð¼~ ïÏ?ÿÌQ—¢H•?ĸ[%À"?"bk¸"b{?Ð2ý›¡²@ÿtHQRƒ?ïjà"'¿ë£BÄ ®¿§ãØ_°J¿ãiÀùYó'¿ÙpÁž›a¿âÇP÷iX‰AGNbcuSUMSS J224042-474733?ïÝmí!Â?b6÷aÎr?=!Ä,2t?-åtWfò?níò'ÖE??ac"4:O?ïØ"3»×?r؄2¡?@"€øì´d?FÙÜÌyk?qÜvw¦`Å?pFg—b¸?ïhœ®n_Q?} ?t5ç+?]Ä{Àë@?_ÖãÕ©?'"'£î8?|&Z£×?ïÁ²À°??\§UåÔÌ?@_YO"ñ?'üóJ¸*?}´¨eÿ¬?[ü"rØË?ï¨YM‰ ?"¤­Tÿ+?V,ÈÓËq?j:'é`?ƒ$ G%‰ù?}–ã?ïšq'¶ÈÌ?ˆ²ÿ£)Ç?O¶«'S{?\È2 DI?‡h0£³dK?†/‹_?î㕉ºr?uP'§ƒ?bێº-Q?\p‡\ï/? ˜îŒ§
?Œ6þÈ?ïRüÅÊ
a?xù¬"l:?S;pZO?DîHê.Šþ?"nӏî?xõƒýýÿAGN4FGL J2241.1-4122¿Í
a"ÀÛcÀMä|"µÜÆÀ;úd­(—À=‹Ydö$@"'ÌGÂ?àZ«n®4?ë
¡äÁ¶?ïÿ ^¯¸À?þ¥nij&å?ûmQÇÈÖô?ï¢b€}¾È¿éªÀ2‹¿áÓ¦¥ñ–±¿ÊLœ»·ü†?Á.èävã¿æ)ù˜Ý±÷AGNbcuWISEA J224103.56-412155.5?ï?,y
e¢?"¼ù´?qçò£Ý&?sõ pÂÞ?" ®Úˆ?"â."Â?ï'9
ãT?–ïSîU?m–^»Ÿk?~eÁM,K•?ˆ|cÑ?*ä'®?ígJò—Œ¤?£8¼"â?—Þ´Ö~"?–{d)"0Ì?­›öÓöu?ž«	"?ì<Tã˜Q?¤Púäû&X?Q·|Aè­Q?XB^mÍN¯?½ÖzòÓÁ?¤J,6ÿ@s?î"S""¶ ?¨E±ËJ³Ü?‡ÕÖ!9‹?‡Y¬¬cc?§åQAÕÒ?¦VJš?îÙaä)=o?«²%‹µ†?{ÔÁŽÜKx?–¶iÛC'?Þ"ÍÚT?¤ÀàÁˆ?ì¥JuL»Î?¥)Q†P(Ç?–s",+L?")‡=–7?µ8ËL¿Ø:?¢ßcƒ€?çÞsp\?ºOôp;­?GyŠ)°].?UYU˜0?Ð8SþãS?ºRԟeF½AGN4FGL J2241.2+4120¿æ`œ ½­ÔÀ.bdä†&öÀ9×Ϗõ«éÀ;ç¼SØÅ)@Bðòç>@n?©c;?¶‹&å#ø¿gï¾d5Pó?²—Ð¸"±@wwZÕ?ëߟ¢È…¿ÌÖÒI¹\ƒ¿å	€¢&Ûâ¿àvé€â"‰¿âS¡2OB¿å2_ê pAGNbll3FGL J2240.9+4121B3 2238+410?ïÝTà4¼(?cÇÌâŽ+…?@6ìòǨ?/6ªù ºÕ?nd˜¯¶?bÛãdŽÉ?ïÛõĽ´¬?rî¨?6c¹ÀŒÉ™?A6`]RüÎ?pžâiJ7?qBõ%{¡?ïTÏÇöE¹?‡ÕÂ_xšø?`{.q3?N@A§¼m?"V¡0?‡x¶¡Çxk?ï;ÇNç!j?o÷ÀÅÛ½?dH;?BeA½gB?•þÅsJ?nR¨­¬u½?ï¹y±ìE?vØüàUµ¨?Sq=)‹$›?Eõ 'þµ?~fØzH¥?u›ÑLüB?ï"KÎ?Šp47Ãzc?MÈh05gï?\°v–érÁ?‰±á(ú?ˆÜ·ZK…?î'yO͞?˜Ù.Š ·?pÕeÊqj?q=L×ۇ?¤½É3Úo?—_'oêû_?íÙ·o©—O?ŠnðŽøö?~ˆæPÓîY?c
gýÙIß?®"l>MµÄ?ˆ.`¯zþåAGN4FGL J2241.3+2943¿ç
-žµÀ91jœV|À:ÂðBóš—À<{""i·T@ q/ÓØ.Ö@óøUӍ?·IËù")¿·ó¡!ù$@Ú~<F@üU8k¬K?Õìmçd'È¿ŠðÔqlù¿å×4ó&Ô¿æä>ÙY£
¿Ò×'™¡ý?¿—Éà´5QAGNbcu1RXS J224123.5+294244?朗r³Ñ©?…ÓYø§™?Bö_³
òÔ?<—¨,Zë´?"+ýYf‰†?"•à&›Ë"?ï±Ù1ñ%?""
ۅ®G?SäZÏÛ¨8?\ÔùLÄ?
("܃?Õß³ÂÚB?ïŒÀ;?'ïÍ.¦Äk?WKÖxã8?cpkG(·õ?œ•Š@`B`?'Ÿ]ƒèÏ?ït@p·ß?srÇÝù"²?S,`f®ž??@œ†Úœ?E<Ýò],?sR~ìjß?ï
léH"«?ž÷\¢«+¶?ZÇñÙ4±?XØøIë@?œ¥ñP@³o?žHÅfˆ?ï5Fq1#A?•,ð·¯?c~wڋ^?rÈ:}±_?–çpóû=b?'LcA?î^¬ôÔÅ?˜ïØ@‹>?`"¬Á/ÝÙ?fÁ¤±NX?©åéãºÎ?˜ñŠo¥ÂV?íı(á?–1²Cxi?r
ÖÙz4?gQWwX?°¹Æ‰âxx?–I§TGsëAGN4FGL J2243.4-2544¿ïÜJ"…]oÀN²]yЦÀ8ó犾4"À;·ÇHÿMS@TXD9ÀÁ?ÿú¨W¢~E?ªñ#
Ì?ÀÝU@w­_I;³@S¥m¼F?ïÿÀà/€ ¿Ù?e*)¿àaâއ	t¿ã+Ñà2_¿çÌéhM¿Ù€/»."¾AGNbll3FGL J2243.4-2541PKS 2240-260?﮿)1bà?"æÐÿ?Tü¡J@ד?[,†+י?°¡"‡×*?"­OU"Y?î¦Q4ÈV?²ƒµ
GÏ?"úýÁõ?§Ÿé?ÏAÕ?š°ÞnZ²›?¢JèÍݎ©?îƒr•–!6?ž@¯Í¬~u?‰D@šÑ‡Z?!á§$q¤?¡wƂ}?¾?˜µì¡Ùx?íIhU÷$Ü?Œ0]I?Š‹³
DGi?l2ÈQ'q'?²cFïè*­?‰{Ñ£Öq?ï'hGÎ1?"´Üxã×Û?jzP"YZ?iÐm'å?—ìô‡O?"PÔé,Ó?íS´l?»æjÃlX? ia·bÔÍ?³—æTû]?ªf"Ûêz?¬õa.'Å#?í£àŠCæ4?¤û"]Œž?–7ù·(°)?"ƒïȬ*?ª¥ú"xǨ? ÀÏ´ç?éºNN±WÀ?£›» Á°S?œ¦Ö´{I?"b®©ñµ?Łëîâ1Ÿ?¢#7kéAGN4FGL J2243.5-3931?£Aœù«;ÀN`:!cýÖÀ:‹ÆÞÀ< 7Ǫf@½ëf?úí@w❪?ÃQsûz_B?¼BÎÜãÆ?ö¯Äcq¿`@E3²_
W?Ŕ€ãÀ.¿äbžÍ¶¿å$¨ Eæ¿æy¦µ¿è%Áۂ¿ïýݱ žÜAGNbcu3FGL J2243.2-3933NVSS J224326-393353?ïå¶3"h>?Y¹…Ü9A?7¼Ä™l©?(XB‡r#?gR3Þ¼©ã?X!ÓÐOJÚ?ï×Mà™Äs?qVCø¸?Cûl›ßß?K[yúH*C?qÙ¢A_¦?nKA¹4:?痢ä‰4¥?p-õ'Àq?X <àØà¾?U-­'?ƒ8¨¾ª?m°ìÍ@`¨?ïºú
2ÿ˜?X$pý¸	ï?[Ê¥ÊbŽ?:c褾6ç?{t†¬ƒ^?V'£`¨Cy?ïºþ¼]?r¦¬ˆþ?IòŽ"?7)ªL?¹.Ñú?qÿŠ¬Ç>Ý?ïuÊO¢ˆ3?TùÙ)ºT?YW¹n°ë¥?bý׏©ß?btñù¯?Ž)ÀÛ·R;?ïMV˜p­E?ƒïüj/ÜÚ?ib!/íò?i«D
Ì°?"(èÇù*-?€ù¶K\…?ïAc[*YV?w[‹*cÖg?qºÚÌ»??YRvêÌøÑ?"e¤-¡m?uˆâ\ÍAGN4FGL J2243.7-1231¿æX«ÎâÀL_9&A³À:pûëžÀ<7ªËñ@žhJí6@‹SB3'?³ª$>®ç¿±±ß‹–K±?ý÷½#â]@~矕¿âu	—Xw¿éxHÞ½¿âD­Cš‰"¿ãS{ýýFg¿Ñ)O¤Øçã¿à³ã'/ßAGNbll3FGL J2243.6-1230RBS 1888?îôýÛ/?½[²6–?]ëÙT?rDæúÎze?ŸžÂ·ðÓ¯?¼­MS‰¯?ï³<]Sm:?4Ëð¡Î?W†'ñh?r\Ì '
?€@·ï/Ï,?‡ÎºY?î÷ÓÞäÒR?†ì|0 ?mÍ&}
M?qàÅa:"?KßOÑçx?‹£6KL¡È?ïDÀ=60?{aPÞK?_ÉmDŎ?F¬=n‰ø?žYqØ­?{B¨O¶ ?íÐë…I«p?¯ãhÁ|,?x×é—{
?tAEÓõd?¯ï¯@£?®s_²½ãî?ï=°eç?›ý¼
IÛ?fÆÂúÂz£?u}+ŽËø£?•q't3½?˜y¨êBÊ?íx—G"Ï?ž¨fZ	Þ<?|›š{<-?x)å$‡Ü?²uÑ¢ÑO?œŒýUµüí?ì¤÷ƒs?œ)‡ãœo?yi«¯¹ž?l¬¢k={b?¹Hí‡;úÖ?œ{P7¸Ä{AGN4FGL J2243.8-2510¿Ñ訁ÔÀN¯'Àa"À:~-o}À<
qäHêU@M¾—@iÒaaCè?ؤó…?ïÿÕm…>™?üªáÀyØ@`œ¤ç¿Ôúҙ•gÜ¿â ç×Nl¿è±¸¿y¨
¿í•
È?Ÿ¿»{šâD¿ïûX0B½ëAGNbcuPMN J2243-2505?î÷ù.]>'?¥YÉÜî³?löGFDð»?r¶ê—øØ?bQ'íú?¤ŠL@<´{?ï‰æ<yFØ?•…Þ¶5/?r-™,?†ú°ÝCl°?"o¤\O?ˆÂ5ÏW²?ë¦Vªuy?ªH[Žq?¨%† Ð:?Ê†3{щ?¶¼ú9Ÿ?¦±6fµ?ï628¯?†GŽ´ä"Õ?Síõõ»³?J]Û9,­¼?œ§þw™Þq?…­øKU¾Î?î·cÙï?°kF…?ƒ‹j:\ €?ÒC0
È?©¯2¬&n?¬Ùµy°+h?îèrìAîH?­äo6z®?ØrÜç-=?šÆá• Ì?šiºë_?£¾qÙç2?ê'pEÀÝ?¬Ù4i]?¨•0Z9'+?Ÿºø{?¿)å¨L %?©ƒ^ø;™?í-w›Ü®±?¦ŒD/O'?hB±<bÛ¼?iÊR~¼ñ?µÒ-•i¨?¦/ù—ÛÿEAGN4FGL J2243.9+2021?ÇêK£"ëÀ@®÷S½À7ìõì€Ç;À;5ìlø@L·
Gç?ûrÀç¼<\?þÞmÅ<?µ®_4ª@qØ¥H#…@.G«æ"^?ËѺÀ/Û¿¹^f'±¿ÙrԞReþ¿ÛØz™9¿Ý¥SŒ¿âpY.oAGNbll3FGL J2243.9+2021RGB J2243+203?ïïP''–?QË|
šF?<ÏI­á¸·?6'\‡yz?Z,¨?–š?N*ZžM–?ïÃðͲûÀ?w¨À/íˆ?MÁ2œêSy?TÒ¼®z.ù?zOrÀÒ²?u•ÿ O'q?ïe½¾*âF?PÎk‡?|ã\?…•Ù;]2½?ˆQgOû?‡#ë¸7xï?îÍ
':"?…§"Ý[á?d{jŽÒë?L?ãÖ|-þ?¡ç¡0ßl?…U‰ÊC±?ïë¦`k>?Z¬ýW6Ñ+?<ÈãA"]?8£Ì¨Ü?`ÀƒP÷{7?WdÄîæ‹è?ï;¨g	Eñ?žÿÿD½K?eðC¦ž;÷?xçÉ©]?•Ìê©×X?UŸV¸lš?ïA@dýŽ>?"Òåbƒ?€>EnÌÌÚ?‰Ùd1n<=?q¡Hˆ±Ÿ?Ž‹—"rU?í¥ÙLK&?™Û휕o?p©ÎŽL˜7?]£¦ä^ýz?±Æ˜·8¿N?™Ÿðôêæ"AGN4FGL J2244.2+4057¿Ü1XÀ/šw@Ý@À7zw⏬±À;3R­Kþ@¿AùŸ"@4ìÁ^ځ?"œ˜ëZ?¸³7¥]È@$©?)
»@ »Çö|?¨+Ø ¿Ýh܂¢\6¿áóìáÀ#ò¿á0%⒱ɿæÉñ…é¹m¿èÏ|_LØAGNfsrq3FGL J2244.1+4057TXS 2241+406?ォyÀá1?s'¢,У?T÷²kZ¢?Wß~?{ìVxZKO?på*&)j?ïצª¤-ò?ïìûF?E!ì<VÉZ?]Z¬
ÂÌ"?qˆm9 Ør?2Ÿ"p?î<,½3Ý? ˆ×Š­ýÜ?£j;þ éÌ?›jmUDµO?'¥ð^>¿?'1Q@@`8?ïçâtKMÔ?V`£øMõ"?2$W"…~ ?*ÀþÙAò"?eÙÀüÖF?TYûÕµg?ïÄf5áZÆ?ô5–èÍ?QŠƒ͋i?I!Tö*CX?yjDEïîN?žž«B3º?ïi[R%?• ×fé>?aBy±£¥?uôŒ	³:?‡ "sQ7?"âNá?C˜1?œ`ꇐ0?–Ók¬´D?–/&ZÈþ€?'¸«òPƒÀ?'Ó‰.±Q?ï»ünê³+?sÌQ±´Q±?E9í[ã£È??Jë¦0WP?ZŠèZ!?sé"iɊAGN4FGL J2244.6+2502¿Ì€ZÅë©~À=‹T~–À:ÆcQÞïåÀ<"PP@líañ3?üðiϘY?ÑÖï»dD£?ÒòõÀáÜÿ?ÿõ²ÉìH?ùÿ¥è¿å÷É?¤…±¿ÑÑðã'pÞ¿ÞçIeN¹L¿Ø£¹bâ£N¿äáâ¾P³!¿ïÿýF\IAGNbll3FGL J2244.6+2503NVSS J224436+250345?ï¿:'°Ä?qŽ2Wû?P[Qu%F?B+‹)pØo?|L ¤
š?p^Wo™¾?ïE§È#Î?‹NSPø?rf°àžk?n| Û{-?'±rô×<n?‡5^›;¼?ïî46φ?}9!ðÑË?zÚ¢Oäë?|29þqg?˜+ì:À	?ˆµyåmY?íªèjfT?ƒîT¥q?‰ž	攼>?j8Žª8á?®éöä"k¸?wŽœ5a?hY8^?ŠŒîó²?`9¼>~"Â?RÕš-\<?ŠÂvÑ{YÔ?€Ì~?Ã\?í©…—Ùûß?«ä5é?ˆN¸,©B?÷¡jδ?¯f'ҝI¼?¨>¥lÁ?I»F?"í¹	)'?¹/ö5¦~?€&œ³±?¢‰‹10€z?ÖÃ/dþz?ê÷yKùÜ-?ž{˜òI?"œüwÌB?€ká¦ÖÊy?Á®{?³Á…?›+ù›€¸AGN4FGL J2244.9-0007?ïN=_ÜßjÀH­Üa•FNÀ:ìj`Æê5À<CãÎq»@VU7«@pÜ¢b–?Éç¨ìMñ?€}:	Þr‰?³¤ÁÀÕ?ÿÞ½:2¬?ï*2‰}ÿæ֙ŸxÖ«¿â^éÐÒk¿äjÜs­¿åcŽz¦^¿ïù?A3|AGNbllNVSS J224448-000616?ï™DèvË?{æbDHO?G€8'íe?9bJ:Ça?ˆ<ÞCÅ?{#JÚ8>?ïš?‹úÂ?ƒw}×pž?`ÒYÙW ?dãx§þ?…L鑪?€Zñè¹?ïH«´Û?A唣q?f0ýôñØ?WÒn'th?"9ŠÃÆqr?€68Æüñ[?î˜>âW½E?M€Sq?lmë6¸'w?OÃN
Ê?¤µ3(ül…?€÷y³õ	]?ï*ڒ:Þ+?'ãÊÌ3Î"?X‰‡ã¶?LÜ,FÙ:?™;NÖ??'"ÄO™©?ïo¿ÛD?˜C™Ê¨?g%sÒÁ¡?pàô²$?š®7R«P?–¤ßò<é?îr6ºbx+?"EFxbÒ?uO¸ðE?mD§@uŒÜ?¦2>ÈE\?'óC¨"'Û?ì<"Äd?›GP,°e£?zü¨¹?mäÛ=¸?¼ò弄¡y?›W"Qj³AGN4FGL J2245.5-1734?ëˆå3ö҅ÀMºõýG¾ÛÀ;Œ8ap]`À<Ô/[7^;@!´oˆÎñ?óÊíêSÆQ?ߙ«¢°™?ä‰ößÅÎ@¦-['Ý•@¸"Æ©r¿ïÿSg†!?ïô…¾Eu€¿çÃÉîËû?ÈíPÐÒëË¿ÏÄãIeú†¿ïöºÂM¬AGNbcuNVSS J224531-173357?ﺩgÔ
ë?•'H«eU?ZÞFä?V?pJÎÍ|Ú?{óºiù9?'Ž'íÑA?ïÈ°wEuš?'&íp€r?TÊE3?í?q|:°cÎ?vu3Ég*?y æÂ[v?îÖ#6b?'ÿ´¼ÆÖ?€…7=€'{?'µy"N¯Æ?œù"2?O²´Ö^?ï$AçÀÌ?€G¿Öò¡?^ŒÕJ#¬"?RñvÃ2r?™ŽõÏñ¢?øIºœ˜?ï¡ûO8™Ç?'ø•°Zk?fîÖó¦Z?e(wœ/}F?'0…»Œ¥?'5$Ú<è?ïTÂ4B|Ò?›ÞÉ;­1?kúý·NT?€GŠT"é?'èYÇÑÎ/?•ÈmCY®ã?î_Ø¥ž	Á?–qޞï4z?~]Ǭ?œ²:ÓP?¦6¼´­9?"[,$j?îÐÛF¯‰?—åˆiø??eUÑÊãÀ'?hrӏ½*v?¬í•-ÿæ?—œ%¹BÄZAGN4FGL J2245.9+1544¿áFùF°òÀBµ‡aˆ±À9ȺÅ­À<£Ä•Æ¦@ 8`Á¥?þ^ŠÏÒ;?ºÎ¬ l?³[;ùç?ôõ]ʶr@
ÌÕHq]æ?îZÌiÐ~2¿çsø :G¥¿Øýç!¿Ü/›¤
᰿ᆚï/:¿Þ!ƒkáAGNbll1FGL J2246.3+154987GB 224338.7+152914?ïøF$sõ?6ðZ¦(Æ
?†¶^Dbq?		)­BM?Kv–ÚòÍ©?5=)¡Ø6?ïÖã@<í?o㱸Òò?>MÌ…p§?G.'Þ‹Ó?s1²êw?lLžÔÂë?ïÀKÕÉÿ?f½)°SI?Q¬ËZä?IŒø ¯?{nâ>ٙŒ?e Íbni%?ïGŽpÄR?nhîôÇj?\¾•t?q?<JBûò?•N1h@Ç?m¤:âÁ,?ïò§Bà¶u?DûA9
?-%Ç­ÂAÔ?Ìôïµk¥?WÀÂý:?C}—ЌB?ïy†k`îz?ˆt;/8Ï@?O ñÙÉá?SêĤÈÁ?¬dL…¿?‡J¢b+sj?ï•z{TD?uázä	ÅË?ZíÂËu?WÈ÷8åc?‡OCɞK?taXü˜±Û?î?fG\¶?Š³¡}t½?pë'Óƒ?Y@°†¶/?­™=ì.C?Š…ب•cAGN4FGL J2246.7-5207¿ÔPW=K†ÀKê¶â—À:ï/éÁÐÀ<E³Æl@!­#>ô\‰?úƍ«?Å<)¦íj&?³]&¡ª_:?ïÊi²KA@˜»ûÄ1¿ïÿÒ†ëA?ïmMá4c?é°Sº'7¦¿ÀãÛ\1¯%¿âñÝ}t¿¡^ÿÝp^AGNbcu3FGL J2246.7-5205RBS 1895?ïó‡¯pÌ?MR`Ë}¼S?Ð_Ĕ^?[Ô-ýÐ?Wd´!³?K¨Š¢¶y?ïéþ¤"Ñ6?iVë\‰µ?-ðÜ"?:hJ̇¡?d'|RÚ@?gZ(ƒ•k?ïwäsî m?…ûÞ¡û+Ê?P¤qº×?IL2—ß?òTãàyM?…ºˆÿ!ñˆ?ï¬÷¡ÙüX?e«šyÈ«Æ?Ae œð7?0‰Í¦rÂ?ƒ«År½Æ?e,K¨?Ò?ïì<‰ü¡.?Uý#"ø$µ?+<[‰zæ€?¿¿ù‹:?b°y;t…?Týƒ&Ò.?ï¶÷jbÓ?"|5_Ò0a?GëÓ ¼ÄÕ?`¬ût¿Ê?€ùÄýuŒ?'ûAÜ'6?ïNº'û"?' ºÃ\w?Sïé7¶­€?MVvL¨­Î?›×*'ç¥?ï]]«£?ïS£Üq8/?€Çy¦3'?MÆח-Ç?HäöjE]?"S»Ó{?€±<"ó‡AGN4FGL J2247.4-0001?á‹9ÌvÝúÀHÞí¢/jQÀ9ÍÊ¢P!À<õ¦	ê@aóA€¨Ý?ÿÖxG9zu?¼¬†hÍ?±©`­Ç?ô=Òä>š@Wëî%7¿êÿ‹ /}¿µ~#qt6‰¿ä‰!S6ß¿Öký¼ug¿ãË=€"¿åv˜B"ÐAGNbll3FGL J2247.2-0004PKS 2244-002?ïÕ*"pµ?^Æyâе?CxPÏDY?1ÖKÒº»^?rûú¬öÝ?\+›qo?ïÖèÖ(ý6?r:,£Vo?Bߕà¨%?M÷ù¨=s?r/¢ß¼Ä?oœä‰ÐKy?ïj¤l‡5?'ÝÀÜDâ"?cÏ¥ÐÆÒ?`L~¨€F?1}²z"…?'?Ì+Žº?ïM®de?n=pÒþ?fÞ74Gü?Grcì3°<?"†×¶dõ[?l%ˆpŽ?ïœH䱁(?uWgª
!'?Xý¨>zrŽ?G9±Èm
®?…ÎПۡ?s',gçðÀ?ï{¿Ñf?9ß%¾ O?TËÊ0tÃË?a˜¯Åp.1?Ž¡áO?ŠëU‹é%ö?îÙs›¥"×?|¤º`ÃÍ?t<M·¦?q˜¸Št‡?ŸÂyÀX¢?‹ä±ZõR?îTVpœlª?ˆ4ÉAo9ˆ?zVËŏŽ?d.è÷T?§o¿dãg?†…uðþøqAGN4FGL J2247.5-3700¿Óà6ÆÀO쿱[WÀ;q?ÊjåÀ<É(˜¥}Ó@+LOŽÞ€@›m´Zæ?Ö>‡$L?¼oU£J?àhÄÓTÑ?ü["ìÝ¿äCt^v­Ü¿ê•êMT¿ã1¾kàú¿á
ÀþŠÓ¿ïÿßHÐSj?ïbŒ•AGNfsrqPKS 2244-37?ïÆWÓ%¬b?t*ƒ‹äù?Al§'2?6ؗKÉ	?z±‰Ä9Ä?s¯l¤ï?廓óFfÊ?…¨`º]'
?`5S÷‰pû?ilj+(â÷?Ï®'"õ=?€åu5l?ïªðPð?Œ)ÓINä¦?w»¡9hÁ?|'X¼•?–[¹´ù
Ì?‡,6؄;?ï¢;ûR5?föðK|â?P
´v•¨?9ôŠ$ÐÃ?…o'9˜·x?eûFÆ©?ïc±­ê?!Œ ?ƒ¬?P—	$v–Ý?E™ތ¾û?''¹1·P?ŽÞw%B³?ïO ™%g?–¬O6›ˆâ?hþåîšÉŽ?z'Ùë&?'ì ´‡Yò?'ùp—@?îÒâ)o?"Ýe#Û?}UÁ¸O?}_ÈÂòón?¤m8ê?'¸yϲ'?îÃÓ9"‹p?‹ÏÿQòJ'?aóI±úay?YÎØ¡¢î?¢£—΂k?‹nø""iAGN4FGL J2247.8+4413?ïb…-fæÀ*'||R`öÀ9ÄÁA® À<iÍ#3â@!-þËøf"?üb»frû ?³,qMB?Œ#nUY_?ڜb6Uýc@hùÔî¿ìäo¶q@µ?ï<›'Á^¿Þ':_w^Ü¿ßîHÝêVv¿Ízƒ~Ы¿ÙlƒKy{AGNbll3FGL J2247.8+4413RGB J2247+442?ïΎL£5"?‡:€´L
?@]™GŒA?GŒQLÛÊ?vµ
óó,?…Ón·²É?ïâ±<<`?rÖ
èÉÌ?6GHS›??Cž!–Üö?júöŸÚ?q=i&é¢?ï
P)Ûh?Ý	î±È?bÖNÄÞ?Y
6{êj˜?›û0ëãÆí?"^9•N¼?ïF_	r;ÿ?qæ…0ƒd?ePkÈè÷?I׊.a+
?"Ša2g4?q9Çù0´z?ï'aù?‹¶@bSƒÌ?YƁ˜iÃf?_g×1W?Œ.Ëʍ:7?ˆü³R#ú‹?ïª%õKàÃ?ŠaÄòáÿý?P'u+ùG?i¼ê‡ói?ƒf4ÐØU?ˆ	ÂRŒF?íÓXÒ –?›®PKÁ?q"M[u@"?h›Šöõ/?°S™d÷n?›JÌ/'Ÿ?îd"ä£Ù?ŒpÀ: ?vçþ"`˜É?e'Í}çm?¦á&îMÈW?‹~êÍ°ûËAGN4FGL J2248.7-3235?ÔP…²¹	ÀOyI@»±òÀ9í|7‰À<iÆú$ô¬@htbÑ@⩓àß?µŽ]ü4™?£bÓd÷?êBlA@\gç'l¿Ð㔤è,O¿ç$`ãð€¿é†Œa!Øî¿èœl^Íì¿ïÿÿ&¦³?ïï?ôÕ÷AGNfsrq3FGL J2248.6-3235PKS 2245-328?ïúoãÝ£?@
¯F"Äž?.PÅÀOµ·?)•D–€éá?=Xƒ¯"®?8~׿ï?ïèâ4=o?p–½ {Xc?:gkͳ‰ï?Xx°‰?cÐÞVtý?ißsÓ?bV?￝(ÍÝ?p½ñŸ`t1?ZÄ0i$ìÔ?_ÏKÜ:;°?yÄ%N&>?m·'ÜsÏT?ïøT!aÆç?2{rš¦â?+b›Á`W?`æŸK­»?Gê¡Gj3Ì?/ú>ÿdq?ïõXmï
©?O•×MõMj??œ>v¹?=ïüþÓÂÙ?Kyçeç?GÏlïJ"?ﺢÕJ0?"Û2u†‹?Hœnv?û?]è³ñ".?›e«9Vô?'®e8Rÿš?ï›÷š€Ê@?vò›±«m?b¡reÖÿ?dntš¹+¿?"Y¼ºQV?rùˆDŽ!?ïè
.$?Vw_ÊKVU?G'¸.Ó"·??h‡¬/?b
ÐÃgvn?QµP˜—©AGN4FGL J2248.9+2106?î£ëâ32ÕÀ@±Å3À:P.ŽˆÄ_À<[6@KAqåK@·ÛnP?³?ÂT¶ø°?´÷îc c?ñhãï(Ah@V0´RØ?ïS³çc¿ßifËæó¿¿ãÊ
æ
³¿à5ŸI[ê¿è¸ê—¸ï¿ïýc¾yåAGNfsrqPKS 2246+208?ïô¢ºæ¬ƒ?DãāGÇ«?0ˆÈë'?+(¶7Z«ø?R˜ƒ÷sLÿ?A-jœŠÓI?ïá¦Û÷b"?l_-'²0ñ?6,±âÀڃ?B¦Ÿ©Ÿ!?k"ãÆJ?i0îETµ?ï¿=#ÂŸ?m`¸ž_N?TºNýŠv?T«#•Ä•?{ZÄۍ—?j׋$àVç?ï¢ÿôÂ_?TÈÏíá•í?U‹hšê?5÷bxùAœ?yK¹#9 v?RåE]çðŸ?ïí%µq;'?R¸qȅš}?@N"7ˆr?5Nú2Ä'?]'ÕÐ?NËÛ±d?ïŒ`
#;ç?‰˜ÖŸ5DB?MÁwf)7?Yé§EÎ??‹åo
²y?‡×n'X,'?ïžMLRد?qFÐ%÷%[?^M>—(q×?QÔºm«Õ]?"£M ?o9aé[¦'?ïd¸"!N?q@•#ħy?iݤ"-õz?QêçÙZ\<?-8×¾Á'?o½¶×‡ƒÊAGN4FGL J2249.4-1300¿ïI²¦4ÀMužèóÀ9<äw
}—À:ô؄ô@ OÏë1@ðúÄV܆?¼^z‰³ób¿¡UWv'Ù?ꋾßK@@½àJÙ?íÊt}€^_¿íz	ç	Žõ¿ÅÄyÇÑ¿é4mÙw¿åCå~*¨¿±ó¸žík~AGNbllRBS 1899?iÓP?ådòhªÉ?@`ò‡âOH?LI—~¹,²?†˜.Ã3‡F?'‰V–¿¾?ïÛI Ä?Ð¤Yõ?Dj?ÙȪr?dďÿvt$?o›ÏÞ¬¶?|®C1\1?åRm%o!?´<£_Æ-.?£v*hY;Î?ša@:Aj:?Òì`i)íÃ?³à^]B B?íÄb6SW?—ýn*U-?!deú5Öì?é!À:"ô?±Ô=¢ˆ?—÷Ï¢¬?î¬Åt­•¿?£´>k¡?RÒáQ§²?P)ïZ4P?¤£j"¿Ñ?£}ó&Ññ'?ïÅ…(Ñä?'À–r?AòxP'åº?U¡Î'ë?zànZ¼'?€·x³`6A?æ7|ò!£œ?³Xö.æŠs?Q¼5?—ËلV–"?Ñ¿U6NÔ?²Î¨òŒ€Ö?éleØæ?³Sù{êL´?9ÚÞ~öëå?4û5ë+é—?Ê@ÐúÕè?³QÝKjϑAGN4FGL J2249.7-5944?è~•CÀI§Ž\NµpÀ:ãÝéTÃÀ<µ&o<Ï@"W'
3D@M++ý´Ì?ƆîFD2	¿Ã~'Î?Çåóö@áÐj?¿ïñüÂ2êä?îAw^o¿ãP¸7åŝ~*¨J¿Äs6X¡U¿ïÿG©ýdAGNbcu3FGL J2249.3-5943SUMSS J224938-594421?ïÌQ¹tð?nö »;?CfŠú˜ÐÓ?@:gé%Ù?wjQÔõ?|?mV13*" ?ïç}»¨Ò?j&F	RzÓ?.^¤9?:ÇÜ?2?f
¶YÀQ?gבv0p"?ïL2z‡æ?«*	Ô?c|µs?c!ûî‰*?"
Ò²3?€kŠG7;?ïãV}©è¶?NŸq1¾ÄI?9Š/sè™?&ºöӂ?ix<†©áë?M€5'Gã×?ï"	(?)RҒ`ú?WÅêdË!J?R6J¨?ˆDø¦œÞ?€X…ê™Ë?ï³Ii{?ƒÊ¹ûÐw¨?@öîª?P貝×ÚÞ?'+ÛÓ{?ƒ\9û›
?î¸W±†?ŒÜ
áÔ{?l½Mäžy?hx¨Ȃ°?¢®°d̺?‹£[¬|‰ä?ï·ª zsä?jBán?JWm¨©?A~ôµp¦?€pªçR?j7§ÙÉÎAGN4FGL J2249.9+0452?íekb‹ÀGJiߗª¬À;;m"XÀ<‰U>öµÔ@ÔBŒíd@£ÿYçÓ?ÁÉÓގ쿦ÆcÉuw?ãkD´e@¿o`
+Ó?ïÿQº÷k¿àšPCrŠ¿ãkâ§)¥¿è»F'‹ˆ¿àñÈ.Ø[¿††="«»RAGNbcuWISEA J225007.35+045617.3?ïßËçt™?aëø/RÞ?3¹Ooû?'69o|û¥?n™œû.è?`\fO¶;?ïÀ¼¨^н?yTu¸gß¾?IÔfxjý?Q½®þƒõ?|g	·º?v"Ÿ'Çe?ïP;.DY?"ñ]x¢?chMGô?ešÆ7*èM?"‹uMo?"+"é¸Xµ?ï¹2îŒ1ž?]ÊpóþU?B/¼0Ô-N?'ö~ ØK?€H£ºJ?]]N>™D<?ᆭAÙÐR?qÍ
Žê?CãlB«?;™Ê–}ÿÿ?~0q†XàÉ?pÖöQÍÊ?ïu¬gÛ7?£ÐŸØ?RÑ3±Ù¼?_ÄdÃØî'?_Å	i?‹a´fÝ~?îË÷Šïu?8¸¥šÑ?m}»·ç…?hvÎö3a?¡h«—ÌN?ŽßzNz·V?ï ¥Hñ®?~·›_†ì?Y—ú†)Ê?M'ØÔãÐ?›rkµä0Ÿ?~ Îú
ïAGN4FGL J2250.0-1250¿ï~Dž)ÀM:'£SÀ7`@ÒX'	À:oîÑ"2@ÎmÚÎî@Ìy1D?šw'ç+{a?Á+±I8®@*ç'Jð¿@!¥r6ð¿Å±Œ)™q¿Ò|	°ÛU¿åÁ£¾¶‰"¿äœÂä¾®¿ç€q¿àÖ¿ïÿôA…ÜMAGNbcuPKS 2247-131?ï 0dKÙó?›Yò\F?n¹Ë°?D·K"–˜?"8—Ø®¨?•gçòwi4?ïa>ØǛ¤?¬ Ռ?r9†ìIf?™ÑÖT"‰?Ž"{2/?¦HÐòSøƒ?å
¬/7>õ?³ÕÌñLî?º0Г'þ×?¥íÔ6&e?ΰæùZ¿?°©SÔq"?ítÇóÒ¨·?«ÖV%‹Ö?kÚl.9ÁÈ?k6ï$@t5?³zìþm8?ªãóþìŽò?íÔ š™Æ?©¾Ý·/öv?ˆ¦ý¦º?ˆ&ÑƞÅ?¬"7
–<?¨ÌEåÓ´?î"?˜j??¶KYT£þõ?'©‹hÏ-?¯v¬M´}?œ"cyÀîð?¦ÄUÀ1ûÿ?æ¾.?i³‰?±³«úN£?´´à¼=¿p?¤°?)á{?ʬ֤ß?c?°/'–tÂ?ç.Ÿãé&¨? "b6Å©?Še…J?.ã?ˆKÞ¼{?Ðϔ
¤¿y?ÁîûÇrVAGN4FGL J2250.0+3825¿äÂ|s¼À2Ô8ÑØ¥À9uTáä·À;ð/Þí@!dèŒñÀ?ûi¥ë·sŸ?®ôMS?'¡Ö\¡Q?ä?O™›G@
}ÙªUÔs¿ìô±d "?ǔ$9Æ_¿Ûguû.ßç¿Ó5dæ´¿âÒÐ¦¿´¸¨ÓsZAGNbll3FGL J2250.1+3825B3 2247+381?ïö…–5¼?J¢ÎŠT?ü0°'?eµsÿ?Q4³]´ië?H¥GrÇ¢?ïèw"'÷ò?l*"ÝMº$?4Ìù}Ä«?B]ž©'Å?dîÍA(¡¯?hà‹(!?ïy¸Ð¢?ˆH!nõ'?XÍõ¬k²?b'€z©i?Žxæjo?‡ŸéŠŠÂm?ïZc¿Ý?po®w˜Ü?V8¹6B^V?8¬µ[‰dK?"Oü‰×Cn?o"V"|%?ïï~'çÑ`?URsÞæ@?-J¨ rƒŒ?$Nÿ‰þ£?]Y¤È2"?SŽ¸åØR?ï»uçê?",Sa=?C¢ª1¤qÜ?U÷¡?ûïÁ˜¸?'ý·l8›|?ïkjÉj?"Ž7þW?]n±sµñG?a
ê«?›»§žZ—¨?'õ<¯=,Í?îƒ{×?‡¼ó"è[u?iUsFÃÅ?S<'ðŸÿ?¦9çw/ýÃ?†Ükì±EgAGN4FGL J2250.4-4206¿Ôð] šÀN–HƒýP"À:"ë=ÑçÀ<æšÔ,=@ñ¾1""@¨Ú!I%ä?³ö¢3F(ƒ?qJB¤Œ´?À"z~K_z@"`d\?îE ˆ¡#Ò¿ã
AQ®ô¿ãL¦ló"¿à‹,žÄ{Å¿ãb¼ÃjM|¿Óð
H´ÐAGNbll3FGL J2250.3-4206PMN J2250-4206?ïö	Ñ(ëË?Am¬óÛIK?#øî"KÍ?[¨´'?Q‰^…á}?@=†å¥¾?ï퉶«*ï?g™xÐk©?*`"^.-?:ì&
æ׸?`ÐGMjð¥?eE)«y.?ïÄ!ë7F?dîFR dþ?L8¥*m]?3ÄÉUþ–?zgõÛ*‡å?dY,/Κ?ï媿~'?F•5_#Ù?6
`+n"T?ïðÇ6º?h-©1˜Mœ?E ¼ÑÚÿŠ?ïí=´Q¼ò?QÑֈ͘t?3T;	?!ÑXGÁ'?`^êo¾?PŠ­>yN×?ïɱQœ)í?8
?:Uö	¼¬?Kú€¨S5?y‡Q´ýÊ?}[MÚ܋ƒ?ï #K%â?rÖÂá
ç?S ÞO9?CãV⃊¤?…ƒ+:¼ä?q™S"ÏÊÌ?ï¸ûrÍD?fyžn¥?M"¾~+…?7õGF¢x?â49Ôª?e5¡_$?ˆAGN4FGL J2250.4+1748? ?²©ÕÀB*ù‡?úÂÀ9ÿI¯vz±À;ü3Â¥@pªEä;@HPïܜ?¶×(˜¿ˆ"¿Ã'~Ó?ÅBÔ{lÝÏ@P",P¿ç%=Ì4¿ëË·XÇAs¿â.LC¥q>¿êaÞËÒÒ¿â£Ó¯?¿ïó¬ÐDÑAGNbll3FGL J2250.3+174787GB 224805.0+173330?ïLñõØ?"28ð&š?APÖÙBÐÈ?8WÍ85ºú?•×:"Š½?"ÇIbñþ?ï­m•¼?€…"Iɶ?R:yÎ 'ž?VßfÞ2/?']K†Ðb?}²
.ì—?í	œ¯VLñ?£Ç­êz?}¥žäï?€ñcù'?µØÀªÐY¼?££]!J&?î«(ÿ—i-?€ì[÷ºC®?T˜¦cQ±?;'°g®¤ý?¤¨ªÑÌÒ0?€ÆŒ p¦?휅ì,}P?±)ËBŸg?_GD–i¯¸?['VnI?²ž³‹$@?°ëÀ€Á¹ý?ï	ÉdYé"?œ-©³!"?bKfs8??jØÚo =?œ}f¨Ã'˜?š^áÖ¬ñü?é™GyÛ?°ÖMÑyó?"Vì°HÛÝ?Œµn'w?Ç0½NÌä?¯úú.$?ì&¤éŒ?žæ$,ã–?oÇ%ä)"?adÇ24¬Ä?½ÐÊTÄÊÂ?ž¤Â‡mÊAGN4FGL J2250.7-2806?È#ÇXLOíÀO¨×ƒßóñÀ8{cRµ¯zÀ;™kŸ‹K@#ëÀ š@cTÁ"tŸ?¤õç"c'0?¸abEšh÷@ô‹"'Å@­ñâÝûŒ¾>êw¿ÓÜ#…}ƒ¿â¨½¯"˜¿âo–[ ¸¿ç+úŸ˜â¿ç+Kb©îQAGNbll3FGL J2250.7-2806PMN J2250-2806?ïëùÚY!?Q3{ÑáJd?4}r¨»½?%¿'^¨Ãy?avw†lfÁ?OÉs&jYY?ïíæ"P?fG‹'q3E?,"9Ýik??É´Œ­ÑÄ?`WIm¨?cÒ­YzA?ïlŒ+ƒ!Ä?ŽL‡¸³ ?sSj}z¾³?d[·k$?‹3?Ññ°?Šˆ¸>lÅ?ïòpÅ\by?AÀ¦9Œ?–ï«Ah?.Vú&†?Y¥~?A
t'nª?ïÕ'ž£¼?f·$xì	-?9uˆ4_?/	ôÚWÿ?sƒHån#µ?e،ovǾ?ïÑñÏ»"–?|ºÆAò®~?B#©ÙXÆ?eu–oď6?tÂ¢ï‡ –?y$©³
M6?ï>Òïâ·¬?"¾ÓjÒÂ?r
QpaÇ-?qÂr#[–?"¢M§˜¸?'CN#îU?ïâ`¹ÂóŸ?[½ÌÓ§E?'É&Ï%`?Kg½|%?l"³ÏöÛé?[Žh6ÂÙAGN4FGL J2251.2+5550?ï'ñžW2À	MÔº.À:·¶'Τ=À<ž¡@W@´n œ˜'?ø­ä	)tn?Ք#c‡?â5ð²…"ê@z&3pp@"u€4ì?ï·²­fÖ?ïû"€«1¿ã¢à՘Mi¿Ô×DÈ¿éeã>~?÷¿ïÿ
Çhß½AGNbcu87GB 224837.7+553415?íÒè+R›?¾Ï>…æx3?wúÀ™AhÙ?ˆ<{» 5?¯Ò%@;.?½UéÁz3M?é̉PÔ·Z?Åó1À0K?q·€Ò#Öû?ƒã+Ÿõ5?È@¸Ê[?Åy€™e?ì
Xö'A[?§zS­L
?—ðbºEœÓ?'?µ	¨?¹™œvšp?¤!ˆ Sñ?î¤Î¿ ?¥Y¶í¡à?'›X"cR?mâþYð^?«BÌH•1?ŒïÄù­Ð?îÖÏ4˜?©#rUDñp?"–×ý•]?"h4¨t¸?©®-\Q$?¦:«´ú?ä†S úˆ?ΓQ
ð?{Àœ9rm?'•-t
‹1?և>¼íöW?ÍëL7^?é2°u—öp?²¬˜A›Ný?Ÿw¥Õœg?•!J­—58?ÇFIp6sÚ?±&¶UW™q?ìšqþ"?¥úU6·Mê?‰žS_A?€³.²ò8s?¼gbQË?¥dƒ}PøAGN4FGL J2251.5-4928?Êõ6SÀLù¸Që…À9ÂXr‡ÜÙÀ<;€kË*5@ ÛçœÜÅ?û½.äïÙA?´$í ,ì?º—ën£w@QJZ—%K@•#"™Þ?ïØÜx5?ÓÇ3{¨ø¿ÜÌÜÝ;/¿Ñà¤.Èë¿ß
0eMŒ¦¿äâO §)ûAGNbll3FGL J2251.5-4928SUMSS J225128-492912?ïú®Ñ}ûG?5C肙×?£sâVZr?n|ô¾?BðJÿC–ø?3±Þ«Ö#N?ïî`I0v?fü"¸#à?,֓—鍽?@Œ»>;?_¥)Çy}?dZ²?ï³xž!i?vQpN1g\?U†õ"±ç?Q.†$@¬æ?€‹"ý	›?u‹}Ÿd?ïיÏ	'?PÈ\äÖ-?<ûd.¤?$Bΐ ^9?rc†Ì[7‡?P‰×`ו?ïù@NµÖÍ?:zuò? ½Ñ-ªzÔ?¼œÓ¡hO?FÏQꛊá?70z¬É¹?ïẾ«ð?UF‡?<'Y]O?H…˜Ì~²u?y/×R¤Ø?}r'/¢?%TV?€M0n4¡?aA=ZêJ?c^¶m´"??‰BkîMñ?~›üROóÓ?金HZ³?j£ÈN:Y?Oâ1:úÍz?@ouâijf?"ßJí}á?i2K1¤¹CAGN4FGL J2251.7-3208¿âÏSÿuZÀOͳÐ|"¶À;6ªw7oÀ<­[.ú¿N@!V\îm†k?üy0ˆ^ó?ÆÔÏ»¼Ë?g"õƒá\¸?ŠÎ¥rž`±@Sõ.jÌ}?ïQ8×·âZ¿ë©Åá¡A¿Ôìò»ÈC¿àUçÈѕ‰¿æ¶b!Z?àU¹pޏAGNbcu1RXS J225146.9-320614?ïæúl~j?_*¾"­¦?)Lð`x?!ÑÌ?y»?hh6°KMå?^Kˏää?ï·Zñyf?"ˆ–uԗ?T÷dÄ.|m?`ð©m%$?6ùjÕUñ?fÖ,‰l?ïL9ôäè?'Ùµ'×/?XsĨÒûÈ?E²{"èZé?"ñ‹FeW,?'¦Fô³¾?ï2'Q¢h?}2@t-\+?N)ä>txO?7ЏÜB?˜¼`õ·r`?|þ	tŒ³œ?ïÊ8#n*f?s¼-.j®?<t^rî#?6ý»{G³?y¨qÁ•ä?rmr3Ks?ït×k>ðß?¡­)è]?XXà3ä`v?fY‰gו?¿	3¾?ŽpBÜi:?îȤGƒ³e?Œ{°"KÀ¸?^šÉ8{n!?Q¬¿oxÕ?¢€å='úÇ?Œ&ÿü­˜³?íU-Z•?š³@¸ÐY?cWø¯·Ø?XQ>=RÈÜ?´»ÕkV?šÛ¾Ý>í£AGN4FGL J2252.0+4031?ä'ó°nüÀ0ã"[tšÝÀ9>Ëò²9¤À<	z‡…›@À'Ÿ:'@Ñ"2w?¯¨Ž¡ebR?¤9¯¤A?ôü…×Dö@	\'»Ô¬ë?ÒÞ&[´[½¿ÓSˆþ–É[¿á–¥ÞÌS«¿Ü|—UG¿â§ýª»*
¿â¡·ªü˜lAGNbll3FGL J2251.9+4031MG4 J225201+4030?ïðü®€ =?Qmÿ^à?/ƒïUן?"<9šÛph?Z$§ý§
?O°žúŒ8?ïãÀ‹ËÑ?q¯~µ¡Ú?<Ô3Bù]?IQïÑïó?iN¼TUî?nøÌX?ïÁ?o£ô3?bNk¸ª¿Ó?S""Iía?EàZv2†ú?z{A:ÅJ?`W¢‡ã'p?ï~èLsåÅ?dÆB?kÿeºê®&?GºIÂ'?‰FiýY?aùìÒwA?ïá.]'ße?b*­ŠöP?C"èw'?7'ƒy:<
?j
½|,‹K?`-èÅM¹?ï¦×O‡§ª?‡Õ1YÒ?Q'lž–²ú?`ÁS83'?"þ•Aÿ(?…Ͼ‹ïÌ|?ï™Í5þ>µ?uʱaE?^}âÜ<,/?b%ïÈ?…¼ö(sD?rbµ¼@á½?î՛p'ì?€îß:?€f¥1š…<?dq¯8G??Zøà?|¼,òI""AGN4FGL J2252.6+1245¿˜Ic'M¦ÀDf¸w«À;<Ÿ1‰À<œ׊•ñ@ lià™]?þúEዠ³?Ê£âëE?½g³¶Ñ?ò"ßq?@@Î*oë¿ïÿýFKê?ïû×ómK?äÜ7£~ö¿çOHÿ΂¿â•Oçžà?µüé=ÝÜAGNbll2MASS J22523220+1245109?ïߟ8-Þ?n¦½,?00—õàqÕ?#2Ba•A~?nåM"Xý:?nWÁœêÊJ?ï½êÐݗd?x:%IÎÉ?LEÞ•\?Rî×°Hç3?}Ûåb?uM™ñÎÒ?ï5ÔÁ@…4?‰;Ê+hÖ²?jéc½øþ?sáÓæ
Ò<?•è;_žîe?‡0±Æ¥™?ï$PWíc?xÍen±Èì?aY‹ÄD??Q	"‰ÞãÀ?™JÑê«Ën?x
'K`?ïÏì@ÒÐi?qÑb_Òí³?A'QYØ?:@"®­9(?uäýp-ºx?q¶ö™>?ï;Ì.—B&?'¦}œ|¼®?`qõŸÙ–‹?n:Ÿô‰¢©?–x;€'»W?¼À¨5ň?îΝÜX†?']í;Å7‰?lOdO¶z¿?o뛃üfÕ?¡Q9}t?'x®ƒ×°?íîÅËPËÊ?•é^&F¨À?mg_®f\?g3üMA?¯=-Nk¶?•œ&ó§¦AGN4FGL J2253.2-1232¿º•ø5—w½ÀM]Ñ_ÄÖÀ9ß=ÍÀè"À;À®J*Æ@*ߊ¿¥@ÚøßzN?Ô€"ØA?á©é"mé@›ç¢;(Ë@à{/Ì ¿á×xø9b¿æ=¸È3
¿å¢Z¾ž
¿ìÿ atd+¿ãHY€NïÒ¿ÐFPܼYAGNbcu3FGL J2253.1-1237TXS 2250-127?ï­QåX'?‰»ñ~»?CjB\Ó?@Œ<hⱉ?ƒ…Byi#ã?‰viÎ+ÅÌ?ï˜.`¡¼?f²ºÈ€?i›¢Ýëy?wš0prÈ6?ƒ"c'«s?…&wˆÙ ?ëÎö[3á?§«ÉÁ:? Ûj›ëˆ™?—!|NšT?¹—Ødµ«?¤S4ÿgÞô?îܑ]Wkn?+٘OQ(?ae)é+¼?Ib.ú»†Í?¡ —uà?€u"¨Ò	ã?ï1/'é[¬?–yß¡
³?Vêio¢%·?V=î5oÓî?˜kthÖ?•æeÖ›?îø'R3¶?¥^œÌE?|™ÂžG–©?È»†ƒ†@?™Çe|é?žA¿È?dé?ê§a×*]?ªK@Ø? ²©Ï¶{?–¦P#hl?Á>‹ù?hî?§¥€Ñ£U˜?ì{¥5rí?¡}Ž•q-?v‰íõì?gP¯ªÇ?º¿SýÙ	F?¡©?:8ÇAGN4FGL J2253.3+3233¿°3;£ÿüÀ8	"‰a=À;-Ëë%À<fÙþ
·y@ 4ÓÇ=@o³·RE?ƒìÁ´À¼¿€Ã@ö¯
8?¹!˜¿/@g‡ÒœÅs?ïù]¹ïzw¿ßmµ»
\µ¿à²ž­›¯¿èòÂ?U*¿àq¹KÈ˿ے¤²ÒOÄAGNbcuCRATES J225312+323615?ï¥sW™!­?|‹ýHóh]?B~Vßk#$?6ñšÿn܌?…{D·˜s?{ÌÜâЌx?ﮃùÍi?|L#hëžñ?V3Ld-æ;?\6h«'Ðà?˜˜<Í:Ü?wßDÞ0©?ï6è*åöƒ?"2ÐrˆY?g7oþù™V?['•]"žj?–<2°u?ƒ|
%Ý&?ïzšíÎòc?eÓ»K?Q%(#LÆ?5(î]nä?5ŸÜð) ?e­€ñ÷è{?ïI¾`›?Ž¾RB¢?T
¥î?N8tµ™::?•Ÿ#"¥[;?5¡/a®?ï/!ÔnµH?•K‰7Äû?c"o°Õ[û?s&i*£Þ?—©WyNû…?"/:ïÙÛî?îp—ž(è?"2;ì‰8u?sø$Fˆç?hVÌ'#ó?¦wŸZ^?'d
–w˜k?îRþýÌt?†úx+µ»c?g«DD†r?U«ˆï?©U[á"??†ÇH¬¤áAGN4FGL J2253.7+1405¿ïZ­åDØÀCîWûi˜JÀ:Îb«ÆÂÈÀ<v²¹%P@ ¥‡4è&?þLhĸ*?ÇläDb°y?À|êŒP[?õºÂùå3Ì@—dÌÞ?'?îϾB'¿íè¡^ßßN¿¸\2ZñQ¿âHMv«X¿Ý&-;L‡B¿ÙvÞ¸1µAGNbll3FGL J2254.0+1403NVSS J225354+140439?ïÖW	H z?móÐaI΃?22£tÐEŠ?-=Mˆ9ÍÆ?s±Q#7­`?mø
À†Ä?ï"h9Ð0Z?"]jH#Q?\ê1$xÏÜ?aóY߃?‡H«tËIŽ?k€67¼?ïNêޝ"?á…QÊ3Q?Qž­B"·?S:§'êÎ?•Ãф=?ìX†¾pu?ïgî´Ý?zÒ3eFyŒ?Uqu1ZP?=ªiÅ4Ñ'?ž{êãâ]Æ?z¥FÚZ®?ï–ÊQƒ'?‰®êo½*­?GÄbðŽ°?A±éÛ,?ˆüGF‡?‰DµU{¡P?ï
€Sb?—ÈR¸¶I»?dcÈÃ{õ?nwUåŒM?œ#|ˆœG?•æ»ßŠVÀ?îˆj‹þÀ?™•(Ô\#?V~šîüª?M_Ûr_ÖK?§S"|?™'mŠ£Û³?ìƕ§,æN?™&ü>æ?j¾õ£ŸA?\–Ëpš´"?¸õ[qµ?™8sRÌÅZAGN4FGL J2253.9+1609¿Ñeht³†*ÀC©~+VÀ4ºaŸWH¼À:›²xŽ@ˇįó@K̼ܔÁ?|gÈ_V‡?¹¬‹cË×Y@C‡~|â@%ᖏùÞ¿Ìú'WÛß¿â3ÂÚۃI¿æÎÇxÏõ¿æÊֈ7q†¿ëa#0†°‰¿ìVB+ÐAGNFSRQ3FGL J2254.0+16083C 454.3?å0^Èjðí?Ë×8çä;?«Ò#¯Ï¿?³å#ý'‹õ?Ò;è*˜§N?Ê"e:lb?×/õø%|?ÚX`Á"h?â*¤ßv?ÛÏtòÆ1?²Š/76^?Â.|Ûk1?ãŠJðpQ?»z²ÎžÞþ?Á_å´¶fÀ?°ÎŠ˜ø?Ð;yÃëþ?º¥ü9³I?~Æ<9•²?…Ë 6|?éæSÓß.?ÁïP<"—?Çp~ÍæRZ?Á££Ö?áѪ£ñÑ?Éq–™¼ô? …ŸŠÌ²?¨@š#'-‰?ÚKöÆù×¥?Ê¿d¯W?Ò,«Sg¨?Ø·ñS>ìO?äâOD`O?ÚiR;X"?°:ÚÖאì?À¶K‡yÓ?ã¶b8jÔ?»LŽIÀy"?ÀAsÓ6sZ?±o´¢¯Mþ?Ðr¥¤¬?¼î'ÃŒ\?'b½ðRZ?'F¿Ûa_ø?➬*ÀÈÝ?Ð÷x•pª?Ú/'ºÊc2?м¡ÐŽ'MIXED4FGL J2254.2+4305?èJ€ß/ó/À-'L¾´À:‹"XÖÀ<Áh¼P@ª>0'D@^e'
?»öùŠp¿p7}¡"°?­xŽÃ8	Ã?â%ébs¿áò_-¿åcŽDÑÁ(¿éÿ½Ñb^¿âíŒM€¼¿ïûS]u&?ï¸d*LåAGNbcu3FGL J2254.6+4253B3 2251+428?Žú?¾n·Â?˜BÖd1J(?¾5H¿¿ü?y#GÑU‹?'9xǑúi?îhn2¯÷÷?±6EÛÆ(³?'Š<ô?¡ˆ¸€62? wW¹ö‡?©iHï¸(3?ìèO¢T©%?¢˜Ó|3™?žúÑòðZÃ?"ú×¼«¸?°þÎnæÒ,?W3'%²?í~¨=1Ÿñ?–̪%"è?œó˜»
·Ã?‡*ûû:RÊ?©›¯Ë¢?‰š]ç?ï^&þhô?®æÍ)Á?""&´­mÍ?®>]bž›?ƒÛ×ÝM?‰ÞÉ#Ÿí?ëўe'Ä?Åڎ›'§þ?¨€ËáM3ü?µŸ;"£•‡?»¹
ÃÜÜ?ÁoDï¦Ê?ì
ùâÉR3?¥Ùb¯¾T?¢u|Ä3Ñ?—&2ø-K?¶mrߛ†"?¡ÀÓ¼¢"?èÎh·_¹_?±ï1U×ZÂ?¶¸'é]C€?¨-Tp-ß?Áj­d…C?©A†&júAGN4FGL J2254.8-2725?í²¦5^[«ÀP	ÿÖ"îÀ:D¶4‹À<,ü<& ü@ ×0;Üúí?ÿò‹ÿH?ÀœÒ^18²?:燎)N?ÐɒZ¶@·{ý+?éý+4¾y¿çª|?ì¿à»²}ì¿ÜP'¤_›F¿â"?_'`¿ÅÑûÆ_uAGNbllNVSS J225453-272509?ïøÖ´	åæ?7éé~ž¹? ðJcã¨?íbƒþi$?H4ÎÊé??5~¯×˜€×?ïèÀHã|D?j(OŒ%®ã?)Vî°>¥?6{éùX<??eªH'Q{?hŒ 0‹[é?ﶞ¯zxä?kx¸ƒ€±Î?NìKw¢?9QXŸzE?€i"¸Û?ju°×?ï¹|häÎ?cHPn´ëé?5w½8

?xPW
é?€õ'áÒ·­?cDNÌ´S¥?ïó³W"'?G¿q©íM?.ó:üL\? µð°ôê?Tºê½œ¯Ù?Eo%l,†²?ïÀ©º	aå?€Bþ8îß?<F]_''?Nÿ–H#Ç'?}æ½4c"ç?~ôëpò"?ïvx,êø:?|-5䄡ª?VØK…?H€¢m؜S?†ò/ÚN›?{‰Ì»è ~?ï('²LÃ?'"÷IJ¾??Må
í4)û?@'z²4Ô?šQ› |?'7fYŠdºAGN4FGL J2255.2+2411¿ë·MYؗÀ?ˆ;`(^ÄÀ93´±M†À<IF"@n[4Ùü`@Ûª€qªg?¨àA¸uí¿Uäa`d'?±¯Û @Ê! c¸6¿áþ3a¬Bi¿áNË?.¿â<8*ù¿áŸà¥Ç¥F¿àßÕó¼ûž¿à&JLTliAGNbll3FGL J2255.1+2411MG3 J225517+2409?ïÖ
$­E?l!YÔÎ/?C»®þ7 ž?@'`íÉg›?r€Oå?i֙ë&;Â?ïÛ†Ñô]?zòF(åCÀ?:¸#Æ:É?HçM¿*?pѱ)ò‹?yzÇ8…M?á¤ä?ƒ¥½sþQm?_¿"÷éœ?lú§üµÕ?‹%Õ%­‰?'¥ŠÖG?ï¶#`rq?c¹•±ÜGE?R¯DFn÷?8=R]…?€!?s½üÍ?aãif^ûV?ï…dOØ&ê?†¤
"ÿ?Y8­˜l"v?QoþQ<{6?‹ÖMIÌâ?…&‡sêB?ï€I	šn½?"ÿđ'€?I¯ôH|+=?ZõÌþ|nz?ŽR¾O϶?"ŽAn+Ï?îì.zDrS?'¡¨ó[?iŠOB?pbõ!»u¼?ŸHí.Â
Q?'ZCÛ[ŒÂ?ïR–i¸¹?€ŸÔ´1QZ?fÝr왌R?U"Ú
e¸Ó?'Ñ"|Y?~{
ËAGN4FGL J2256.0-2740?ï«Ékˆ(ÀPýŸÓo~À9<çƒ1xHÀ;Uù†i;-@åBÕ<²ä@¡…÷%f?´f~«<ë?'Ÿ˜6B1S?ÚÔ֜?@	ðÖ. Qo¿ÝŒZ@é)O¿éÃÌÞj"¿êˆì9ò¿êŸ<¦y{í¿ïÿtN†v?ÇÙ府mAGNfsrqPKS 2253-278?ïûðòš£?9ýïü¦ÝÃ? Xûb³ ?#óa·¯?8R‰4Ý¢?5G¸È&?ïÚád"X3?vR¿PɂQ?Gëkwywî?`ÎŒ_j»?o#ÁP?q3é©3åë?î8#SRs¦?žáÀx e5?'d"Òa$?‡{ŽØ?§ä¦
ÕÁÊ?›ÄÒKu?ﲬÃr?må³ÎÑP?Gˆ"—Sºr?5ñBáëÔÝ?ÜMKÖA?lȚúF÷n?ïðl…å2?_±3¢B'U?6i'2'ïP?85Ÿ_àÁ?ZVƞÔþµ?]«Lkg?ÇAÑ?'ËAð*îî?]S¡†ð?m$ûõrË?ˆ«	;t?ŽäÏ¢êü
?ìåÞ¿q"5?¥uáÀe ?"ZKk‡dB?'{w‹y?³úw(¹.K?£R»¨|?ï-™»[G?Œ+í½´á1?dì½ZÏf~?_Èén"8†?—¯FØk6f?‹Ræ–{AGN4FGL J2256.4-7119?ã*®JÖÀE~p\‰mÒÀ;~à^zÛÀ<âòŒyöf@""'y´¤?ó§®ë:v?ÓmJ[BñÂ?Ûpmü1ê3@ ÀŸ—à\@õƒÈ!{?ïû¼PíX¿æá¨&$W¿ïÿïXz?ïÿÝ/ñ_S¿ÖA9†3‹H¿Åüº¦.¨_AGNbcuPMN J2256-7115?ï™ÔÂ1	Û?"Å®Yöê£?QŽÊ<‹!?RQeŽªFH?‡Xö&½wþ?ƒæýÜ)ƒ&?ï˜àÇ´É?ˆ·úä0Â?b.€K2ç?v˜!U*uë?…<-òpd0?ƒ/!kçã?íé1^",j? Æþ	n?r>+åÜL?v°b¾#,?¯%$šÇŸš? Ò	A…!?ïJ¢ö"Ü?""ó2|Ö?Z=$¶£U?Sïî3%¦–?•É¿K?ƒ·ÓjoT?ïLeˆ3Úg?—üÇÔNþ?e{ö-2,?d‡+Íý?"ÃîOpä?—y-aŽÆ?î®ÀõJ'Á?±ÿ>Õø¦?€ödGh¤x? mi¿%3/? ÖW›4ˆÐ?«Þ–GÜ`ß?í"Øãí‹ð?£ãQ}ˆ?t%µ/C?zö°Íõ
=?µŸf…ÚšÍ?£‹ÿœ½#?íoV›SiE?§8Ž`QÍ?€EGonº€?ˆ%ÄÃe†G?²|¢5´Ì?¦%C /-<AGN4FGL J2256.6-2011¿è¬'ðˆÞÀOr" ٔ[À9cÑû	öúÀ<1¾Ûrþ@Ìâ'q	@À5¤'?¬˜ßàOáj?šgà9B?íñg™T@D
ájÿà,RÚš¿ßECÁu֜¿ãy î?
¿ÜEíhMÇ¿æƒ_—±¿äiM š)aAGNbll3FGL J2256.7-2011PKS 2254-204?ïyIm‡B?‡‡›*Ãl	?VÎÔNJ_¥?K&O:{´Þ?Žà"
Q'?†Œ†Øߛ?ï"0òS4?¤¬kNõ´â?a~ؓ£?tY¹a€?†Ô
S'³¨?¢¿—Ÿ¸Od?í¸_ÁËUÃ?¡Ó!êOXr?}£æ[a?m&eA½­?°bËpç?¡r…N/¤?ï,µSš˜?vº琤?v:a¸9
?[o\îfO=?"Ú½ =k?síàKºS?íëÄ°ãQ?«¨˜Bµô?sí>ZüI?hÜ 0_äÚ?®ß·HƲ?ªîAѧ?îÕÐA©÷?°R)F	™?{…CÑ?¼×Š‹¡Ä?žƒÖvµ71?¦Š˜*öÒ?ì
På9™î?­=ÿŸDð?"É•_Î×?'@ú6‹+?¼üF*9m?¬(mú‡Ú¥?î!¡E¾ã?'Y¯ŠjÔ?Š·LPô5Þ?wá%5=?§8¾«V?Ž4™‡‹ÉAGN4FGL J2256.7+1307¿ïY úO֜ÀDˆŠÅÁ@À;~d^NÀ<5·qñµ@ S‡QŸ¯?þ+£!h0?ÐKÍ=µî?Á•Æü(Z?ò-žž¼J@žx±A«ò¿ÞÁÍ_™Ã‹¿ÎÀ¸Azsº¿Ø«hC`Qú¿Üö)RáP¿àVÎþÖ4U¿ïÿóÀ¬ƒAGNbllNVSS J225624+130541?ïÚþÜ>"Ë?bhà(ö¥?4´`# ¾?%`òœû^?q5KÙÆ@?aÅZc=Z?ï±p®úåö?}³­½/?QVŽÅï?Z
ÍNý?y^Kû¯?yœA¬U-Ž?ïˆ:i»ä?p6Œì#Š?ZçÝXçöê?F^¡Im™2?Š õÄÂÜ?oœlºïÒ?ï \žT?ra»cÈAB?W›²µ¶¼?=ŠWºÚŒ?šzÂ̕ZË?r¡S°Tê?ï¸u«Žõ¸?rQ֎Ðék?HÉÞÞ<[?=µ4ÍiÕ?€`¨qƒ¼í?qe›¼é½º?ï/ó'€Ã?'kÃbE?_´Ï©ð¯£?gŸ"d¹X ?˜@µ™ù?`ÀbšÏ±?ï0øJKu?èÛ ð?cµ1¬Ë§•?\ìÏIEm™?—jPV?€Ï6¤Kã$?íœ"pj*?K›—+?g(
ïc›ø?Wøð'
?²e¬¢\?êök4pAGN4FGL J2257.5+0748?ÜS¦‡áÚÀF¿ŒâÑñÐÀ:֟vRl´À<n¡¾+IZ@X>A¯!ì@'ìCŠ™L?Я¢šÛ¹?¾1ì'9ÿ?æÕL}‡\@«QȽ/¿ç8"Üû¿çwk§^¿ÓàŽ€`ãp¿ç͑¸ú‡ñ¿ïû5`4>?¿¦Þüz9'AGNbllOY 91?ï™ønçu?}T²&‰?P<ÛÌó¤Ú?DüÌ©(+?‡zHÉÜþ)?{±¹‰˜¬t?ï¸Fƒz¦î?zb]N®ô~?QÃfãµ?Vâ
†Ì¤g?käבì?v'o²ö?ïEþ´Gè?²¥üuÔ?€PnÇ{á?'GX¬×?"¯	!Ϥ?""ùúWt†?ï"P|š/l?dÂóÍõT?SùŠt%`?;ýóòáñ?ˆ¬¯š
½?cz¶uä…ì?ï"âþ<†?h÷ÃÎÿà?fVBABs?cē=ð£?›D›Vig?Žî}úì?»?ï8ØÄQÔ?"1ºF¿*m?`ý79ÜQ?f
³{¯±.?–á§Ñõél?'Ÿ=ِ'?îP)m.#?™ñ[íP?‡Pw‡c³?ˆ×úRl'?¥+τÀ¢%?"ñº†½ã•?îѤÀò¬Ž?…£Ï˜þù?d;"'¿qX?[hÒªÆã`?¡¢Åm?""»IAGN4FGL J2258.1-2759?æçüýRaÞÀP;0"'À8=RpæÀ;Sß'Bd)@ ÔûðPà@L…0aÈ?¡€Å?î?ÉVEÜÙ	q@#–žš@¼à€ø¿µ¾!Á¿ÛFËÿ€¿åM1:Æ¥¿è(bTˆîQ¿ëOý¤-f¿í
òl™†NAGNfsrq3FGL J2258.0-2759PKS 2255-282?êa¼ïò?Åàˆ!ö?À2žÖÍà&?Â<|eµ?§?hށNK?¯Ät3~ê?ï¶t_µA?‰ìÈ^¶Á3?[šÖï6a?r¸>ÂRáQ?}ßga?…çXëÞȾ?è·Èµ!E±?³7õu†–'?Á£dzJ,?¬Ù[=¢Õ?¶úñ^û®¥?«µ¶a/Ù?ï«Dˆ+nT?s;ê´5Ɉ?\"Å¥¯³'?T‰'ƒÂ
?ª…6ό¨?oÄâDó—ï?çô;Ðx ?È·Îkû?ÈÃÒI°Å}?ÄoÔ¡Ç?­¬ùα«?®ÖÞ‡;F?ïdO¬ ëï? ºÉ•åÎß?h~¿çIÅ?
5}+J?rzŠQï?œ©	õþô?æ˪–t©©?¶dÕ:n5Ê?Äb¤0åY?®õîɄ?Àn±¦"5?²3D܃/?ïàûWú"?)ÿiyf?sßWôµ?jq>g_â?šÌ
"Šdh?Œ²»ÆÇúAGN4FGL J2258.3-3643¿æ1ÑuöH¿ÀP*0U2aÀ:–…`ýpÚÀ<¥šàÁvW@V¯ÂÐʈ@š"ù$D?ÀlrYŽ¼œ?£tå㧸I?ãm­¸4T@	9Yèԕ¿ï`ƒ-FŠ(?ïòI~N9Ÿ¿Ü)ªu[Í¿éŸKT'(Œ?ª›ÈüfK¿èW'[åYAGNbll3FGL J2258.2-3645MRSS 406-025483?ïð-÷mN?PbŽ#ðÒ?1eyɌkA?$vö'L2?[L{ 
K-?NJs+Û\?ïì÷ȁ—"?d~Ïô¶?*Yþr[:O?9ùùìu}p?ab—‡˜%«?bc‰‹x?ï†H¡"t™?ã0gÚ
t?\Té$h?dþk`
S®?Šílðè6À?~è,›´¼ä?ïè€;=‡?KFStA³@?&Ú<ʎÓ*?ψ%Mrâ?f ¹¿ñö?JQ±Uæ°?ïݽ£#d?b&bòhê²?EÍ!™õ?;+'«| ?lϨÑpL¦?`3œ!¤º?ïÄ-êk?€9x:±ÿ,?A7"äN‰?QT5Ùûg?{†2¹?~̐iS?ï&A"s†y?‰UF"VA?gú}'ä?oå§zU?˜8¾Ë.?‡Îš}%aè?ïÄ®ƒ"'G?f‰—G̟?:*HHB>?2öfҘ2Š?| î(8?eÅT'',AGN4FGL J2258.4-5524¿ÜçCÛ÷âûÀK;Oag#À:aƒ3%Ç:À<¯
@Ë¢*@ya¸âÔ@(a´Oþ?²ÓÁž‡Á¿¬§i¢Q?úPŒû%¥¬?ÿÐÈLŠr4?ÄÍÀ"!¿çÓ²ßæ¯ø¿ãÔ%¼R+F¿à"ØÅ0 ¿Û]:É)ª¿æAž¥AGNbll3FGL J2258.3-5526PMN J2258-5526?ïÄÖ¹5W?qnš~?Pº)J;äc?=½k"!ø?yf
éßÅ?p+ØMÄæó?ï°Óé1îv?~îºÓΐ?Ur›Lzï?U9]\x?(—fJ&?{³uZAŒ_?ï`¶éX7?€aßZW?k­È'bé
?qÙ/aŒ?siøÝõ?yáp"¨Ã?ï€^'i|?jþ¸	¢½C?jäè#¡º	?Pâp˜Š¸?‰/"÷0…?h×c	ғ?ï~5ðWü?}'=a%²?g¸ëCt%?XX³T#ð?Š"I3!Uë?zŲkÀtý?ï1/SïZ/?"œp52–õ?e1ÆÔÉ?k-r‡ç}?—3Ü«†
ó?'èiY
w?îèV"ûéà?‰ˆ7èÚu?vÀ_ÎÁ?s¡q%*ç?Eo;é?†¸"bA!?îi띌1@?Œ…ñ8jiP?†dN%€VÍ?ugFYWi†?£È2œ%O?ŠgÔF­}AGN4FGL J2258.5-8247?ä̀
É©úÀ@¶ YžØÀ9Г¯tÍ1À<4‹ƒVa6@*wB+ɇ@¥ ¶Xí?»]7ÄB?ç-@÷Ý@A¶Ô=—@:«C:<g¿à.'à¿ÙÈõ<WŸ#¿Ú!(¤c÷÷¿Ý{ñ½òêC¿éEÚÍa¿ãdeጢAGNbcu3FGL J2258.1-8248PMN J2258-8246?ïVa¹-ˆ¤?»\Ôèá;«?'DÕôž
?»Ïæ\ÀË?gw—éc?'}.â;(?ïÁ飋úŽ?{
G2—Í?P†ÛBÚ?XÁÿF£#Å?zê̎üÄ?v™b[y¬I?ïª'ZÚ8"?} 5ӕÏ?kâÈCq‹?v¢™äíPã?}]a!³z?s3O¤"?ïL!'] ~?oXì9~mÆ?r¡ä1Ó?PñÇØò?'õå:züÖ?løÛ,Ú?ïÊ@ÜFÅë?qyS‹æ™?qLÿ
ÚH?k핐'°\?c´‰ï^pn?Zá™ ?ïJ8
ô›"?'Sü"ßóý?aîÛâÏa?lÓãô†ý?"{"Ń«'?‡Ú^àL?ïg!?[œ?ˆÂA©N¶?z4µÃ¶˜—?€Ï2šir¿?‰dˆÎlË?°"ù?î+ H[Æ?‹Âöׄ®?‡…zÄ:ƒ¿?oþ4È?§lœÉ?r³?‰9nd `ÕAGN4FGL J2259.7-3549?íõ"À³SÀP05~gÀ:zj]këáÀ<•ýÉÄÛ@ì&.6Ÿ@ewmÏ?»¤ðñ4‹¿"ž/aê›?ØñOƒJø¢@žëq}›·?—¿¸€ÿ2¿¿èWï«&\¿æ>´`šI˜¿×wR|¤–M¿í þG™ſĒ©ei'>AGNfsrq3FGL J2300.1-3547NVSS J225941-354846?ï½Z?q*‰ÊNW?Yßψ'Ó?MbÌ׎ª?{/"4?n]=ì?ïáÂÿ)Òs?pS¨'?9˱2
ê?E="lšV?kŠ'"ƒŒ?l¤ÃRp¥?ïy³˜m¤?}1'ùAí…?lCa°rnÊ?q®ÄXÊ?Š'A‰_K?wY…~@å?ï×÷÷"·?Pnº¸@*j?NlH֛<?2'Î9|ø?p6{›?U?MÝO—Ïœ÷?ïiçK—ò¿?…dçxY3÷?p2¦:zÇ?`¥þ4Ù?x"¸Ï¬à?ƒ㶷?ï¢oÓ;j©?ˆ*NE"íí?J±×š¨§ë?ZOìÈñN?…¸í¬GDƒ?†~¹Hªvˆ?îö˜
"m¾?‹ÖgŸ.U"?w§è߀k?zqû«.:?›C{S¢-?ˆîˆt('?ï"
†–²‰?nŸåœÕá?eÜ'.
(?S€oÕd›Â?…Æ[|OM?k²ÞHÿAGN4FGL J2259.8-1552?íZHTâíÀNå‡?úÁÓÀ9ùqÆùgÀ<`9»°è@7/
.­@DJ9ßõž?º+œk[?ºÿ"JOY…@µ­é¿@b?Š.˜¿Ò¿žÁ÷‡¿ÜÂn$ïß¿ãbåþL À¿à®°³ ¬¿äŒñ_Ô&¿é¨eå7&ÞAGNbcu3FGL J2259.9-1553GALEXASC J225957.26-155332.5?ïù†+}²2?3Ї£X"½?B"êŽz?
8ü¿} ?F–''?1²¢Y¹Bà?ïï¦ÖetE?e¥j7Í:ø?+`û‡B?=Gˆ"Ty?]F3"&–É?bù-¤67?ïÌS	‰¸ó?YŸ?wñrƒ?Nü}l ?6a"ý—í?uöël'ªÞ?V"+ß»ì?ïÞÍò«ry?IÀE®¡šÅ??§³6¥?´?!MKûå?m=ú´?H#迏¨?ïõF"«q?A½Ïàþµ	?/³8ìŠ-Û?Ɛ"ßX¯?Q|p»jSû?>Á˜ú?ïËL9áÅ?~d¾ÜV?<oÂ-«±?Lr⳨?x®]בÃØ?|!tÛúˆ?ï¯`Ž=Îu?iË×Épòê?V ´ß#ö,?EëS0œ	?SÅÔÿÙç?f¶è'§Ôè?ﱤBȅ?d3¨of'v?Qè}™g&v?=Vrj³LË?YߜÁ—ê?bŕ~Š}%AGN4FGL J2300.1+4053?è¡‹wå6À1=³(é-À;4½çXÀ<œIwBV½@":QŠŒ5ƒ?÷˜ƒ$"?Ó¶, ð;?Ñ5@Ԇ€?ú…dÃÎ÷I@õ˙Fª?ïpŽ• ¿ïúS] ;?íÒ ¶ÄLÌ¿¸úÕ^@Ó¿Ð9*ƒŒ<¿Ù?͚'AGNbll3FGL J2300.0+4053NVSS J230012+405224?ï±ÿá?~¢¤"($?DUÔº3J?:fŽ
žù?':ª{@
?}õÃ>ð2?ï°OK E
?‹,Ž†ô"?SÚpÉs«c?`Zsƒ W?pßOkH?Š€2õˆžC?îXSo­{½?™•ÙrVòq?cP¨Œ˜)?n4;å!Ã?©IÃýÍ!?™wÞ]îÈ ?îÆ\Ô0?'§¥W\B)?O!ÉjA?:ì¨è¸õF?£¬H©Ú2?'"¦`°þ"?ïvÛ(°?"Ú0'xŽ?[}Ζ2R?S†ž³h†?š9L¬õÐ?"*fݎùÉ?ï;[¶4/?ŸR£%d?\|îþÛ?l3&ØbÖZ?–Ìǯ±§æ?ž©¸yhÞ?ìê–Ú"?§=^¢{)?`Õ<½2–y?c
:SK?¸)5Dº­?§´XÇ^«?ìÑw¥í©«? Ë@'Ž¯Ó?Yü¢Ýúïb?T¢L¾óû?¹PEÕ±ª? ·®½È AGN4FGL J2300.3+3136¿ë4´döúžÀ9'ê>xâÀ9'üaåÎÀ;øV"ŒÂ@d?3F©]?ûÀ§$œ—?´(Ùþc´?Ãï$eü¸@cÈ}²³F@Qä&?ïæªY~?×êdbU4»¿Ôòñ#Ä*g¿Øj'ò"È¿áæïÃqÚ8¿èŠ.A±ÑAGNbll3FGL J2300.3+3136NVSS J230022+313703?ìè·u2î?µíp,ú?ª¼íÒCÖ?¯¯ˆ®º¾?¬d†´±ðJ?©8—žˆ9÷?ì‰L@º8?»=
<(¥;?©àòkc=?°˜í»ô|-?­ŠIˆsÒA?®	ÜÑ'?ì /q?¦"C£Ç.£?±z
ÀÊÌG?¡ÇD#zÁ?¬óð|O<ñ?œ<v'úp?è€êY¶»Ð?£Œâ.¼^ž?«\Xˆ'»R?ˆõÏLcG?Ç%@v'®n?¢ªõÚò[?é6)
yß?ºhWϗ$?½œñ׍	?³'ã±"žÒ?¸±Æ Ђ?°*ηgó ?éüÏQ"ü?ÃàÍ­ì=?º¤-Ç8Ž<?¾røÊEwÈ?½#ë†Lá?´Dýd^I?êì¼:r0Ž?¨ý_.Iú?µÚGÄÂ?¤Í+ŠzöI?³—Cæb3Í?ž/ܐ?ã
ÅÈÃö?°ÖŸñbÞf?µÔû­P~Ê?žV­ôŠúò?Ôu5'?±·ú@™kAGN4FGL J2300.7-2645¿å ³ÍnÖÀPWæšÔ,=À:ݲ"ý[
À<{k%@áöfÏÿ@i=¾§p?ØOsûÐE}?ÙNäH•@:ßdš@Næ¤g¢¿Ü÷K%˜?ý?ìԝ¡;#˜¿â~\&qƒÑ¿ä‡ä€G¸ü¿ïý~E€<ѿ䈴€ÈAGNfsrqPKS 2257-270?ïÞAÁbص?a>¸,ð¹'?J¡"ŽÙ'?@­g~TÉÐ?kÝf¿Óó?]¯ÒR_(É?ïÞd¡rß?rïc€{?@©ß±YÀm?N. é*>Š?mÐ#"âÜ=?oÇ}H{R?ï&ґª._?ŠŠ® ©?u™(7'?h<Ff?'já<žÖj?"*Ú39«¯?藍*'ùè?d$1Éé¬?Xq³«!"?BF4¥‡HÑ?ƒÃ‡=íâ?bä<ÑÓ?ï¾P_éʉ?s.Úû!?_ì´!óÙK?Uxðµì×Ë?xÜ¢ó}?pP'-%)ì?zç&ë?ÛHpÿ?]÷Ë/0?yÐkïè‡Ë?"zâEñ+?‡w£)Ú&Ï?îÛâ_!?'8WøI?"ã¤.ç×½?ƒ¥Äg$Ç?šëkǙõ?ŒžâÄã?ï1S‡ðŽ?}Y;¢çŠ?berCÒ?XQžN¦S?—ˆëÇDêÄ?|ÉϖÿAGN4FGL J2300.8-0736¿³ïfX±"ÀLªt)ˆ<À;1²åšùìÀ<¢f®ŠÂf@ ÔÏj5þÀ?ÿ:o¸¿ß?Ã÷¤;Þþ¿§öO¨ó?äëûѝ&?û²{诿ì,¸Å®ËZ?'¿FÚãn'¿ã®ÊM–‹È¿ÖÛt/|ÅM¿åÛ;à€Þ¸?Å£3÷(kAGNbcu2MASS J23005469-0735438?ïà'Æ»³?_ÁG‹?pÒ?6³€'·ò?(ê^³?l¦Ée¶©z?]ÍÀ©Z,H?ïÁ¥=*?{`p\ç0?Rs͸C4?V¥ŸILsM?zÙ9éÄøî?w.^ÿ)?ïƒKGC†?wƒS'©?\é3uÑP?F!¦ÄIÇ?‹¡>f‰?vÚRT2G«?îÿ[Û¦Œû?{0µ<}ØË?d"˜§ü?Jªló!‹?'‹ÅOé?zª)‹sùè?ïźbG?k˜£/."ª?Eãã% «ð?7Tç6sef?zfD"[Ù÷?jýCT?ïQÜJæz•?"cŠÚ]/æ?b¿°"]ûÁ?lñ#ò5*œ?"l€Š=«é?'rvó"û?ï:G-ÞW?ƒ ÇÎDÍä?b°–ä+?[NM?–azõI?'wEÁ16y?ìàN¹˜ßØ?š2:
7¹?|·j{ds?nY8^Íâ?·2#W|?š3ñk@AGN4FGL J2300.9+7108?Þ)¾í]ˆi@$XNaŒâÒÀ;B* dúVÀ<¡'~Ê
{@ íœøž·¼@g£Àd¾?Ö2%™È"?ÝMŸ$óÕO@0K!f'@F2"QÜ¿ï²BÝË!Ò?æ÷,Êx?ïÿ×ñÃý¿Ú°ïáú±b¿ê\Ö/Læ¿ÚgC›‹6TAGNbcu87GB 225907.3+705409?ëuß>®*d?Áð!£ò@­?‹¼À%¤ž?…^½Õ¬ý÷?Àxg: ã$?ÁÆ8¾¸b?ë~¥5jVF?Â$çbq²?œ'úya?£E.<©?½%³î¯v?¿¥n¨Ãó?ë~¢j×?¨­¼7ê'3?›'²ÞuQø?'!Ÿ¾Ê÷"?½*?ï"1Ó?§&øô:Rv?ìêdµ1?šL£4
~?¢[)æ;/l?'EÏLkÙç?®þ"¡uj?–-½"–Ë?éHÃ-«?Ä1NŽzÎö?¡†Û‹]j	?š?%涱A?lj(­ûP?Ã5ŠN?èxâŠ#Y÷?ÆúÏ`¾1?­½Â`ÉÇ?´¥Ùæ 9o?Æ­@JŒ°?Ã5jÃËÏÕ?è¼ØnI<h?­@!ß{?©ÂVÁÌ¡U?›@G/ô¢?Ɯ–žßÌ?ª¬+½u?èz¹ŸsxH?³N=T
7:?²Kî¾T³?©6Ž(Ö?Äï"!½êÝ?°ƒSŠSoAGN4FGL J2301.0-0158¿ì¡ÉšïÀJÁ—¢H"ÄÀ9KþmuNÀ<͆00I@	('Ö¶@ˆ+輜?°ðZE›À?»{u·O¸@S;wG@¯ga8)¿¿8¦³³v¿á垪Ðy¿æ½}h5ž¿æ†yKD!¿éïj¼6|"¿ïÿîbHÊtAGNfsrqPKS B2258-022?ïçÌ[Ò}€?]CÖýß3?8%Á	(mÚ?-͜jÙ7?e.ì«{?[.×JÖp@?ïèvŠå'?uvãéI\L?2J¸¡ûʈ?C€	=[Öù?e@0@˜?t.øâÔ®?ï ß'噚?xsácÞ§æ?_œ %w"i?WE	¥•XF?ƒÔ¢¡C2?v7¤8nØ?ïõ}ÑÎ$¢?8†\ƒPÎ?GxÔßM™?	³+9÷o?Säš6(?6»Qvùª?ïȁŠÈà?qlӌ]\¯?EÎ{ó#?8Ä3ãVg?yk=ªtL?p¤'¨-—?ïÄq
ьœ?€¼'K¾?I('wÀQ?cŸÍ7CI¿?z¢jQBï?{¾_¸q—?ïGuþðò'?†NÜ
ëå?m³dúTq?jjtÿ"«?"ZӞÉ2?"7ãCIT?ïèLQ"™?TgSV4?2ÛÀx
6?&6þ(|îö?e ;Ç4'?RÜ®1x=iAGN4FGL J2302.8-1841¿Ñÿ‡"ßJ©ÀO×L`RPÀ:»¸/†ÖHÀ<¡Èê¿üÛ@ªòêí¿@ä"]?v8?ƶgZ­³?­1÷㕪æ?åÌÙAÐ/@]tWjÊú?ì!ÙzZ9¿ä¿'Bd(Ÿ¿àüö•óò¬¿áï;â"D¿æZUÖ¿ïÿo˜AGNrdgPKS 2300-18?ïÐÍÝemº?{:Y¡*N?EËf!£ä?7bŠôéVS?tߤœ¸®?z†ßXÎÃ?ïÊVèïî?tX6k' %?Kòe‹'•?OëpÃø?wV>ÏîE;?q¾Q€ñm?ï‡ÂuÊ¡=?t'"ýÍð?bfò4à¼T?f{ß7"?‰u¦~Š?q7F#Œ?ïqúƒ"J?fÛ4²¤Ùo?cp\S{ô¶?C3ýSÝÑ?Žß*S'â]?e²Äæ1ùP?ï¡-ÐPm‰?zI0]†g?Xb×UD1?HiÏà$?"¨J@ÓË=?y_‰ái^¸?ïnê7'Ü?©Å{û?\ÝWo	Æ{?fIs
.|?Tã è‡,?ŽÓ|w€¿?ï:©=j]†?}*»\»V?i§ÉøÑ÷P?b­âó?•uß
Îi?yæ‰}"ð°?îŽrô`±é?ƒÔƒã?tbÜ38X?_ˆ×ÒQØx?¤Œu1Äîé?ƒ#nî—ò(AGN4FGL J2304.3+0618?ì•ëÀGÙmã2iàÀ:¢iÿxÄÀ<`FS¡gÄ@¾
0•5@úxCÞ|"?Ï0Æ[ïj?ÍGÇêºÉj?øc×ZÅHt@
å+|…Œœ?ïþ~ÀÐ?H¿áî÷. &|¿è™¢¨áá¿æð(A<¶?¿ïÿ¿h`;ª?ïZZ¿i6ûAGNbcuPKS 2301+060?ïÛÅk(Ý?"(,5Ö
?7x¡Ú°»?1–~M!?p¥þùy?"a'"C?ïºÏç´Y¹?{ÎZ f?T†º?²B?Zø:yяÄ?}v]¡¾"²?vâÈNÈ@õ?ïmmóÜÚ?"É‹q/9¡?ljܱ3 ¹?p©–?³¦`?‰Ì‹Åh?ƒˆjîC" ?ïÍ9O"!l?Wfë¡?L¦ÛþRñC?2äîÈpU?uÎ|¨Y¿Q?Uoê (?=?ï×ntZxz?qÑqÆòQ?C.ò‰–ô?B,ËQ·´?qâ灴¦?qBõ"—~?ï=ßÙÝ^?"éðSw'Ö?ixÙZLÆ?{k»½>e?•#uËÀ$¡?'­ȅ?ïÝZtÑÊ?hî€ü"¼?u^&?xÞ70Ø_ß?—¡=*lŠú?Œ57wÑÎ?ïa-m1B?wˆ³ŽQ'Ð?b,í+ž·?Q uL?'"°Uç à?uý{µ'Ò`AGN4FGL J2304.6+3704?ïish}À5¤]AúvÀ9"n"2QŒÀ<XÓÖ¬@ TÐó"?ýpoiDg8?±—÷-š?}ÅmáC¢"?Íè¤CÁ Ê@
/¬G¿»¦æÿ(¿Ûl¢ Sr¿åï¤"^¤¦¿ÍEþâô¿ÔÑ{ˆ6šÇ¿Ýá/ÅÀiAGNbll3FGL J2304.6+37041RXS J230437.1+370506?ïöé|—Ž?OT÷uZ~Ù?­°@儻?¸˜Cuy?P²+ÄÓ{â?NSÒ}@þ?ïîDz>›­?f·{ Ã1?(KføŠ?:°8mDŽ¥?`6ÕÀk‰t?dÂqÚîc?ï{´Ç-¸?†`¢'–¿?P&,\?ï?;,ß	p#?:¨ïh|?†?1¸®Ù?ïÖÆË"u?RÄg—°;?3¢ëÇ_þ?êyo
?sbxrìÑ?RV'TG'K?ïíËú-ÇÓ?_›³-[?,Y÷ 1ÇÇ?'/–TJKÝ?`nf>;7®?]X(´+ý?ïÊÜp‰T?€ŒÙ}[?6¹5CY¼?G´
þÔ~?y1LyvÚ?¾‹hkà·?ïw÷?›¶ÉW?V
l5Jt?W†ž…?šÍxH…Á?ƒãUΉS?ÓݕÐ?n¾£×D§?I{Õ3æx®?7° PÐЄ?‡?¦Ê™<?m4¿AúAiAGN4FGL J2306.6-1105¿ÕÃÊOnþÀNMêhìSÀ;+š8ûÊÀ<¢RÃò2¸@ü%4ÂÕR@éĤà¹?Âìv¶?Ž¿œ«ÒèUûp?Ü}Y\'¨?þdÐTÖ×?îI±Y¤·?æ*¿ëò¸ࢿÙÅ» 'è¿ÈO8·×rB¿æ®"2Q‹äAGNbllRBS 1943?ï\e.ä?—‰'ˆ9ˆ?Qøèés۟?K
Fš?Q?"S˨6IÑ?–¿V¯žš‰?ïĔ‡È?zTÄ©ü)?PZ}þ°Ë§?XâÝ{_ã'?yŸ_¹ä?uëê^U
_?ï
oÑZa\?~ƕ·H?dhé) &?aM£ÝØ?œ$è´ã5À?ŒC2g'Ün?ïk6‰ÒÒ?uÄȔd?\·îÿ´¤
?JÃ}Dƒ¥'?Í¨¸ó"?t-ù‹ ?î°åè—[?¦.{1è8?h6øC•?bë0*	QÚ?£n@©›?¥—n&fU¦?ïzK‡à+?'^–'E¼Ž?WÓͅL
;?dF·¾U<?Žr¤J=4?'D
†e?îRvŒÃó?—HPù--)?kƓàåŽ?lbÍÛb¸A?©5)}]ì?–e³úH$?î5ǽ2??'¥98o'ü?uÌU2ðl?mÀ`â"o?©õqw4Áˆ?'+ÁŸ©nAGN4FGL J2307.4-1206¿ï2ªú¿ú+ÀN°µˆãhñÀ;JÅø5À<«¤¸²@ Î
ŽÞՎ?ÿCýrr
?ÅGQù#¿'ŒÛñH?ÐõêÓH@Š‡À©(?퓿e=W?áÅÂíOú¿â¦ìq­Â¿ïÿêf:Ç|?ïÿž{€©ß¿á¨Ðº%*AGNbll3FGL J2307.4-12081RXS J230722.5-120520?ïäð©/U?iíŸ
Íw/?0DÖÌe?1ïŽ't«?iNNxþ(?ip†98[?ïÀm
Óþ?…CRüVq?V>úp¯Ï–?jEϹå·?z9ºmC	H?€,þ_œÀ¼?îågPK`?—"+¬±B?'Ew††Ü?ˆË6)ÅG?šHs@§U"?‡Q2
"Ç?ï»5vÀŒß?orhÖ@?Ä؉UÙ?ÖVÒú."?Ž4‹?nàå
³Á?ïÉ͘Ç,?}@]Ý
´4?C8Îfu?De©2"?x²æ۔¯?|öWš!¨?ïyº»Ÿ ;?•9Sæ?]¬!Xß?sû<Ä?ÛÌóLä?'B§" ïÂ?î#Oãÿ*?–¼ â"Ê?ˆîš›Úãý?ÄOEz—þ?§'äX5Ÿj?'›–¬¦Òí?îÚcdd"»?"Ñųg›Ò?7Õì3ãÅ´?@YÉõ\¸Å?¢*ßß°?"Ë/"ÁhkAGN4FGL J2307.6+1451?är#ó>|ÀD…Å3À:!ó¥~ª*À<*¬3Ð%@AÎ\
m?ÿä̝Òä>?Ä;9ýQÏÖ?Ì
ɲ'@¬Á^ڀê@G¾Šß¿çëi~J‰¿ç¡ŸÒò¿Ù:€™îS/¿âßN_¤¿ä:aûš°¿é{bŸÝVAGNbll3FGL J2307.7+1449MG1 J230734+1449?ïò	
Œ[?[‹‹è?¿À?:à˜3U[F?Tý2
ž›?U5›ôaï
?L˜%,ˆ?ïçaa+?h~àÙꯛ?/¾<ð{<×?;ºMA^ã?f£¡å›å?f³0cä?ïyCh¾
?'ØÓBi%m?k'Wcei_?pDNd˜*6?ŠåOòÓéï?€"ôÈӑ¸?ïÈ÷"îÃ?VÚjn"ª6?6Åù±ßS¦?81jŒž?zÖzé\Ó?VZ~Äè?ïìÙî¸?TÑ¢xQ&¹?El¥-ŸõÚ?;pjpÙJ?\Iùùù§1?PÇíÀ9wå?ï­Àâcb?ƒ~ýÒ<?BቧwO?V¡¶h›@¬?ƒaΆË2±?Þ'Ó¢?îñ…*·È?'ݽ¢òº›?zâ=°ab?|R­ÀxƲ?›ËRâ­?
*I]¡?ïk®°"Aw?uð,ðÃ?J!<	¤¿?9Ç" gª?'¹ U?uÄ¸êiAGN4FGL J2308.9+1111?Çý›G׍ÀF)Q֌i/À:¥àªÐ"ÃÀ<uý'w>%@öª'».@(…ZGt3?ȎpÜ.1?Ò«3À ìà@3Äz@a¦ˆ›p¿ïÿúŒ—Ó?ïÿÄ}îB¿á¸rØd°"¿åVõ°å_¿ìnç©Çå¿°ûUvT4AGNbcuMG1 J230850+1112?ïz§¤ÛR]?ŒãT¶*?l¥™A,¬?d6‡Ax~k?Š,°}¯ÚÙ?Š®ße¦"?ï±VQ£ê?ÒÎ.ê?W¨ý¡>?]‡cxØ©Y?€Ù¨¤å­7?{¡pלG>?íìbŸQ? cd†ðÓ?"Ý%S"^	?'QÑ·uÖ$?§KC\a"ô?œ?vTs?ïv'Pí$Ó?h‹J0Û?nâ³Æmñv?PޑâhYù?Š¢þÆdÀÙ?d{T÷"ä?îñ":QW?•±Œ+QOn?"éž@$º?xɂì·)t?™£ë°|Z?"AOâSb?ïö&•ô|?˜ð~HSƒ?m
JóZ^?sº[àÃP*?›_ú«F.&?•¦wÀ¯FÐ?탕\"K?¢JH§Ý¬?•d/A›‡¯?^>?°ä?­'"}ç0? øéF'E?a뾑?'øPk¢ÅM?5öz¦Õc?j.Qp6Ô? K®ìE?€Ÿˆèª'AGN4FGL J2309.7-3632¿ïP¶)$ðÀP¡¸€®À:&AؤmÀ<rÐîš}@Í;­*E#@,™»þHp?´ '§7¿•ye»Vê?áìi ,°¸@¿­QÝBf?ïþÖj€˜¿ä\º:#è¿à5ŽÂ¦^¿Úr¼€Nnù¿â'—|ˆç›¿ÖàÀ48ñAGNbcu3FGL J2309.6-3633WISEA J230940.84-363248.7?ïÄ<!ÀÏ?i¥êÿH4?DS– 	\í?5>¶pø$?{W|h±D[?hI¯¬l?ïÍf=E
?wh¹Y'æ…?LöÂ"ä­?Të‰ÀbÐ?u®ù/§?s¥ùp¬À?ïEhqzãî?"啥×?gV*|%û?`}ÊBRV?"qgÿXp?ƒ}µ2q"?ïR‡OÑP?pYØ3ÁL3?dÕQ9Þ:	?H^^#¢?"ký(À?nç{µçe?ï…v£*š?|AIc…½?VšQd"x?G午¨>?‹Ïö'ÿ?zó"㲤{?ï{§`Ÿþ?ŽP"_Pš
?Yó_Heû'?bôZþNà?×»ñ»Í)?Œ%žÀ·û
?W€]?'Ö¥œ9åˆ?sÅÙù9?nÿñpT?£LßHþ¶$?ÒeŒ"—í?î/]Kh;Ü?‹0m\ڐ?zئx8ñš?e8»FIÚ?©¯z0‹?‰¥‹u!gAGN4FGL J2311.0+0205¿æ"Æ`÷çƒÀJºÇË)À9n‹îNÀ<*ÀY!†@O²(؇@Üðû?±'®*?¸UW༘Í@HçÖyõ@'~k)¿å•XA_›Ç¿Ê1V?Qпâ*È˶LX¿çy]ä☿ߺ?<¿ë…Ð>qT×AGNbll3FGL J2311.0+0204NVSS J231101+020504?ïö[¿"0?C||Už—?Ý{ç¿Q
?˜u"ò?Qª©mŠ4?BxU)cR?ïéiê:­?hKV"~-?0'ÅÑÝX[?<¬–Å£¶À?dƒÝìÌ?eµ)ƒ	Fê?ïŒ
Y'û?"å`0[+d?i?À²|²`?u3Ñè7Zä?†­y"ØÊ?è¢¼f é?ïï	q)C?BR¾?$ð#E1›·?YQ€í·?_O¦kÐc?Aj_þ/n:?ïï}Ø?Q0	§°rù?(ÂR‹÷üú?£…-i3?]í­ÖÂ?P!‰oÕ?ïÄaŸ4ì¤?;FÎïZ?@¾s­°9A?T¤yçÚ?{·b
ݶ?€h²?ï?]Åì<?Œºš×B'Ã?n¬iý¸
¶?rV2™×?">Ï
ÏÔ?ŠÌF!ôÞ?ïגÙ6µ?`–%¯³ªœ?7Y¡`õé?'ÎjV…k%?rÀùpøó=?_í3›u(VAGN4FGL J2311.0+3425?ïǦ*TEÀ8煵·À7Òv pMpÀ;žq—òÐm@ò E>y@ëDå^³?˜lð÷¬ýØ?¸YaL1‡@nƒ
áÛ@l7ñ³áï¿´º`
±Ä^¿àÈÊ^³i¤¿å˜9²©5¿å&[^u6¿ë¡ê Ðâ¿èç=@Ó.çAGNFSRQ3FGL J2311.0+3425B2 2308+34?ïÀ`uê™?t~Á'õ?U׸{&x?Ṟl¾Î?zY×Ðɳ?rLÆ6þí?ï×&>Ðl·?v²Â•}^‡?E2÷@¡7?_0u¥á?qƁ̣Ó?ts+` è?ïP¼?•,ÛÞÁ?†îªE¢ò??‹ùZXíÖ(?"o¾"t?'`­øÔÆ?ïùJ¯%Çæ?4çÁ…?)…†´»Ãù?xŒi¶:?Dsá÷M?/&•s94ý?bÇJ'?…ÇÃËÔ$?[§¸¾ê?XlEÉCóx?‡Ü´Uî°?"Š-êǘ?ï'|›ÿFê?'[Ó2T?`œ¨<«Ÿ?v‰÷ñVڃ?‡YñÒ¯~¢?•®O¦?î«Ã®½´?žÚ¶'ÄZ…?‹Pçiª?d?@[¤f]I?œß"Ý?™­³Zt'?ïðŸý¶Ð?P\¥_"ü¨?;‰h?4ompڇ?X:¸á$?KÌAÍIAGN4FGL J2311.7+2604¿äÿ¢¥0üwÀ? ˜€"åÖÀ:)Ö¢8¤ŒÀ<Sæ
ær@®¦xÓ{@!§ýàk?¼m<ïI¤d?©ÍáʵÆK?뙟}^P@•\Tê"?펄'¡WÔ¿áPž1Ú¿åà iA¿åé¯nî¿ä¯^'AcM¿ïë»MlšAGNbcuMG3 J231144+2604?ïóהÀ±?HçåáÙ?$UM²—‰?Bºô|?Wm¦Ã™|?GÆõoz‹e?ïæ¨H3'?l§íSÜÊ?/õ‡|2/]?;»¹ÅL?gX_"‰q ?i®;Z%½¸?︐O÷l¼?p²æŸX?XŸL—£?c?·=û€?}¶"¥Çÿ?kbþz3jÃ?ïæÿ–R?DçÙ炖?7+2CøŠ?Î(cP_å?fVé®ø?CÑb–?ïÝS ;d?cE£vÚ´?8ÔªX3›?+»'›Bf?o'ʁ9Ħ?bc9¬>—?ï¨F¡Ëe?"|P-u÷,?CéalO^5?TÍ	:í¸ê?"¯Á¢léó?ƒEÚëI•Å?Ï2á1?~4¥P,?bÇ2‹ò×Ã?\€–+¨Š?‹)?C·?|ªøK‰¡?ï¸ÙJðO?eaGÇ#?P'CO!/?8ÁVOÔ?o.j°OÏ?d{'p",AGN4FGL J2311.8+4541?°¸Èx0;¨À+}´í²öbÀ:ˆþ{À<4å†×õö@»›¢|@|ôètÉ?Çï­7OË?ß"š‰®•?÷ï~Þ,p¡@×mŠNÎ?ؑÃâB׿âÈñ EØ¿êI
Z[–)¿á1‰Ÿü_7¿ïÿø]Ê5™?íÕx™]4AGNfsrqMG4 J231144+4543?ï¤AQvb?‡ÀCE‡Æ?qýfün?xÒÛ+¢¬¦?|ÅrÏü
I?€õû¿³o"?ï'Á2š ?'ºšMÒ#?l^¸ŠßP?x8=€3'?ˆ7ê'3YE?ƒ:ë5?ïJáÆëª?'`Û ñÅß?t'Úᓞ?u Ç;a¯?'ƒ©Å?{"Iøpú?ïhol8QD?r©˜ƒ?nˆ}zo«á?S&Ï¥TÅÍ?ŽB¢Æñ?nÈÁ]Ù~$?ïaéKÚ?ŠÊKä'?|ðéh52?~ŠUq,¹?‰‹Í7²?0"ECèÍ?î}Lv˜t?²¦2¶	§?'ç!|œr?`½$Ñ*0?£¥Åï/o§?±Y Û,a?îsÝë-5?"÷àô7z	?"gkI$6@? ÍýÔN?£¨F~Á0t?ôÇ 
?íüxkCo?'‡½¹±?‰ÊâD‹Ó¼?uƆ¾sä@?©ÅÀ»‡Û?íÍ¢;RAGN4FGL J2312.5+7241¿ê"T¢]|L@&xaՈÀ:Áñx}ÀÀ<4^[Õê@Uyqk'@{¹Fk?Ȗ³á‰9?פõ'Î{ù@¶l£—I]@¤Ge_M?ïÿï9_J¿ÙÃSÜöæ|¿â§§^~:™¿æ……t¿éþ	ù~¿ïüÓ$Õ¢^AGNbcuCRATES J2312+7241?îÈ.›
³?œ>h‹þ¨?p	ùTÊo–?vðó±1͘?¡{àÀ‰Ù?š0Þ¶?î]ˆÚ2a?°¤& ;?€lM
(wb?††2œzîŠ?¦_"P—?¬ÌçsÈøÍ?íµä)¤'ð?œ]©Êy?Ú8‰ùx?ˆš¬`"
+?¬4¡#O9?™óJF‹?îs«Úg?~ΧGI'?~ǛßháŽ?]Žì.Id?¤ì[OSà?|¢†Ÿu?íëð*8Òs?¦CL}SŠ?wè¨T"w?ƒŸmÚt?®Cûˆp(;?¤—G¨âÂ?쒑›¯"¤?¾$ÐÄÔú?•0—rĜ?¢Œ
×
€b?¶M\C»?¹¼¢d9?ì›óW"Ö*?¢GæPYô8?›SLàÑÏ?'eû?M‰%?´K'¢ô¹?Ÿe÷ÈÒUô?ë`d‰—mð?›¿'«®¨?•7âë(IÏ?|dìüà–N?¿®âùVe	?šJøF¯./AGN4FGL J2313.4-6922?æÍ¥d>:ÀF²SCsóÀ;Ÿ]ZN*/À<ë{o'V@"³u†iæù?÷Ϧ©?Δm_ÔÑÔ?ÍG,å;Xœ@>;¤ò@åÃèL°¿íu/¢/k¿ÖB²A±%Q?ïü÷"
í?ҁüœÌ¿ååwÞ³Õ?ÓPúïIúAGNbcu3FGL J2312.9-6923SUMSS J231347-692332?ïÖ`Ëá".?§q?]cŒ?:µ-¤%ßû?fŸó ­&?s$Gãþ?¦ï‡T?ïÕM-ž?rՕð®¦?>FÂ>]€?Fïöå>t?sxdñÁUÐ?pê­
ÂØ?îxŒ›PËA?›o{‡¬Ä?U%,çÁÿ?Q1í44³¼?§ÎçêÁr?›cËïf±Ž?ï¤áí9?pŸ–þ¡?=´BEšæP?1'é+*ÌQ?…ÚtAܞ?oxmÁ á•?ïÙد6Âg?s/PH??ÕÁ³¬#ç?J) «^L˜?qLbÑ%ã?pĐÕ?ïƒûâ†iÞ?‹0¸ß£÷¾?PYdT+Ù?_M`GÕ?ŒõÚ×	cA?‰q<LDMÎ?íãÝXœ_ƒ? ÈìŽ N0?X©à¯þ?`•¬e~Rú?°~m»ÿ¦è? Ê7ßÿÕD?ïÏ<"¯?ŠzŒ¿ê±Ò?Sô7WÉ*?T"¯¼'à?æØŒŠ?Š]I ÷ ¥AGN4FGL J2313.5+3945¿ìÆ[žâ-ÝÀ3U<¼M#À9³¨eå7'À<!ܘòª­@½sßrl@=ŠT'8T?»òÂ?U*?ęÎØþ´@¨«ÕÜ@@`äƓ¢µ¿ÃÔ¤¯ò¿æl{=ãæD¿é¬MÑD*Ò¿í(~#qt¿àf6`]'¿ðAGNbcu3FGL J2313.1+393587GB 231102.6+393314?ï÷×"CÕJ?KP¡;ë5?6ù®&þ?0É®ˆ1Èë?E–ùЃ,‹?FjÝç
§?ïíVVñà?h{»9íñ?-íÑÙs?;œÊ<g‰–?`ÊËÚ TÚ?f}VcU7/?ïM,J?"A¤fÜjë?p+•õ3?uR='•'?™pÜJ¾÷?"ŸÈð÷?ïïy×KD¼?A"ÊçLŸÃ?0'Äà\ÖL?Æ؎K5|?\ç ¸œ¿?@W`‡÷øA?ïñnüX'?XúêT
°ë?E¯ÙH![ì?Bë]ÆM?RJ¿ï¥²?T/áÆH—?ïĹb.?Ñ?€¸Y‰žy?N;ç¡Mª3?f!ÌñÇ@c?yÛÑÙnIH?~½Ä³d?îa	v»? FÂ2õ2¸?|è Ó,–?~½=§Ç*?¦RT'|º~?ŸwÚ´™?ïʏIà?dL®éÝK?LØpq0×Í??cŠ£˜7?wMTñ?bIE8WVAGN4FGL J2313.9-4501¿¼Ï£ä¹ÀOÊìë¯À:R€;$À<FÅA¾q@½UzþÂ@H.D¶é6?¼/©Ýˆ\?"Ö^úiñ"?ÐD4¢Éî÷@dÕcIP¿æ"G!ý¿ã?¾&@Üi¿êù­ ·›¿ëÞµbLü2¿¾"V7$¿ðAGNbcuPKS 2311-452?ïá·¡R±º?r˜dیÜ/?`0âãôãk?nMç˜ðÇ<?\.÷òçÔë?[,•jLo?ïÞ*ɓm—?s~o<
ûS?>ܲòZ«?Q
͔¼Ù?mùŸæ%=›?pLcÛ¥{?îÅv$R"j?"yüˁÄ?uÿw¶,?|vKÊýiv? è»4ô?'Ã(²qnè?ïíVëF'?Hç4¹O'?%…¬ÒÝ?"Ç3z£‹?aP¹ïæ"?G¬ôáo'?ïÏ{
ëÉñ?wBK†;›?i‡@cɱ?pmÂ'"?fýô
ÌU?i`–«(?ï¢ÀHHÝÙ?‹9P*P:Ê?Pß·õZ?cOÖUWbw?…LM»"¢0?ˆ/Ýϛ¸?íeë-yϔ?£J¯8­¿˜?M:™L£b?FŠ»sË·?²¦ÿAØ×6?¢KîË7;û?ïÄ-»òVl?iʚØZâá?EŽ<–g.(?@ýoŠ¹Î?{7Zvü[:?hƒGº(+UAGN4FGL J2314.0+1445¿êçoD¨ÈÙÀDôsš¿À9¶L¨O?À< >ÏH¨@ ajNÚY?ü¾ú1‰æ?µίP7?¯Ø\"Ó?û½CÂÍoŠ@JÆ!âÔ¿Ø°îŸÛR!?â盺Ü	¿ÞßÑ ïcÑ¿ÙT)McÓ¿ÞþGï¿Ö›;$™<}AGNbll3FGL J2314.0+1443RGB J2313+147?ïÑC†yf?a@4kt¼?BêÄ5‰iO?1t©G5ª?uänŽ"ç?`-Ûè?ﶢ'ÿð³?€?ù/ÐSõ?T-ªõÄã(?YrÃOC?£5‡éÉ?{Õéu¶Ð¶?ï_Zãwg?|Û©9ÄÏ­?eÏ´r/?YÆ"8
?'ZÈÅÎx@?z˜µôd/›?îgúá](?}–Ù¯Ê?x©×ô'ý?Wü$W?¦‹›‰%?{ÍgyN\?ý]õ?~öáÌ¢Ö:?` æÉ.ÿ?SX+­a?‹VQÍ%'Þ?|&Ê	Ï9?ï5'šS°?™†Tr'û'?aàl6Ö?iˋ¿öTw?—+œQÒ'?—ÙâË@ú?ŽP:U?"_´¾l5?xL"Ý'Õ?qñ³¼Ó?¤\t|KW?'æ»ÜºÅ?ì^ëEïà?•~0U´ò£?‰TÌ¥kÕ?p÷Ùs)ês?¹äß#wºˆ?"BvsÙÿVAGN4FGL J2315.6-5018¿»viO
:}ÀN?Žâ†ruÀ:3"_ôöÀ<zäÎKR@×5›J@N_œGÉÃ?»ÐßoÖk¿B'Â%™?К©#¥K©@=tю'¡¿ëåN¾©ô[¿Òe­ÄHﳿæê~Ž{X¿àµâoÌ@¶¿îÌaË¡ÿ?ÏÁ¡
&I–AGNbll3FGL J2315.7-5018PKS 2312-505?ïð´æ²ý?MÕð‰îñ?3/…ÀsAF?$æ×(—G?YËA{'ñ?K'ìô@?ïîvGQo¬?f™·ký'4?,â¾îFÆ?;Þ&¹Ä}?_w׉o?cõÓú9&È?OÚô?"ÙºL붵?oÖ8f÷"?yuæIÀ$]?"§]áä_[?Õâ!¬"â?ïô.æreM?9™ÖvÇ~¶?+"€ÐmW>?¼üV'ð†?T/£0o'6?7Áµ#âV?ïÜ[×Rrû?sKc뉾Â?FFë$ô?7‡]¹õ/?n¡z\<?röz*Ë~?ïÌm^}8æ?}'yM9á?;¹'ò–ïž?N©öZ'éÅ?x
¾D¡Ø?{¬5…)4?ïm÷#~Ï?…ÇëUgÕ@?jßb̶ûø?t»ªjÁ!Å?ÊeERe@?ƒ™)¦|?ïßr¦]×?YêQ_ö?D'C`?5Õ÷ft8?k…õ:
ÉÀ?W˜Ë†Ô[AGN4FGL J2316.9-5210?Ój`ДoÀM­ÝiÓÀ;)û¤P¬ÁÀ<ÐÄe¨Ñ@ T
$Ç	¿?û¡Îl	=–?ÒÑE= ó?¾ùÝ?û\q?çt/è%ç?ÿ©F«
/Y¿æ5à¿ék×3X¿ã¾+Ÿ@!®¿Æßjßÿã@ä̝Òä¿Ú½†þâHµAGNbll3FGL J2316.8-5209SUMSS J231701-521003?ïçôהM?Sú¨«š?(R=	ÙÇ)?&
¨ÕÆî?f†Ì Š#?S ¯ à–s?ïÒ	sWvÆ?uMêc÷y[?BÑZ*-L?Iac'ØE?t¡ä@E?s-æ®"zB?ï…â$\??oÉZK­Ø?YHª$Á?AÀ¹´IãP?‹WØÀ'?nS…¼)ªá?ï‹´!ô?gb՞šš?KARÂaÅ
?4~ï":E?‹ˆ½¿˜Ðª?f¹òä;cæ?ïÎÿÇBk­?k`ñ£AR?: ¯¿»z¯?01CùÞ?vÞNw(v?jæÒXd1Ž?ï$÷?ˆÆt%é4?SÄÌ{6Ñ?bf¶g‡W?Š@Ýr]?†µ6Îü°?ï-á¶O'?~ÕËv§üZ?`,žm§ì?NW4¶V´H?˜>5e›?~²ˆSM;?îƌ/½v²?…+‹èä­?Xƒn7'Íç?NI«zQÂ?¢Ó!ù€î?…Zã@ûŸ}AGN4FGL J2317.0+3756¿ëoߣíÀ5GvĂ{pÀ:ĚŸ˜·À<K¯)M×#@Ñ·gµÇ@AËÚ^…Ç?Ë´ge¿Í`?¶­¾,0
?æqËtÝø@ížÏ
™Ç¿çæüÞãOƿ⸝Ö?<V¿áF%žu "¿æ°Ì@Šß—¿ïü•aütZ¿ï¾áÝU03AGNbcuB3 2314+377?ï½ä =[?vÒ"<
?Oêtì5a_?@Ã	sÅX­?}`ùQ©ƒ?u~Çë?ï¯L?¸k†?d®'Êç?VÊIm¤?]u…uò¶Æ?S¦Î¾òø?~ÿõ&á?ï69–_ä?†ë¾TŽø?t»ÀÚ'®?uWÿ»?"(ÈõG'?ƒ Ž²ã%?ï#o/Ûn?t3ý)z¼?i¤ö¶'‰?L⛉2ºO?˜q…i»úO?rüÎéÐÈ>?ï"20"™?'HMÇj)˜?d™KÙ°Ö?[ñ¡Ð?™)†ÙoêÁ?'³íKÖß?ï0j£YX?œsF¢"¹?m*7ûÃ?|v;vȼ ?›j
h]w?šJ‹Õ»Ò·?îW<°ñ‹.?–•@á0©?"O˜€'JL?WaHîÔ?¥xNÓ9"?"°¸ì†?í®ŠÐå‰?'Í'H
?}Fp'~"?nØî¦rK?°·BpÔ?'.A3vAGN4FGL J2317.4-4533¿îD´° nµÀOâI@¼À:/e‰Ç"À<Vè³³ @½EªI6?ü¯§r 0?º2€…Ì];?ÆǍȪÿ@'3@˜™is?ïþ.~Ãq¿à2÷~|1Õ¿ØTü܊%¿ÝTVc¹ã¼¿ã~¬ãù9<¿é^­'*AGNbll3FGL J2317.3-4534SUMSS J231731-453400?ïòGØ©?L<-"I¨ê?<g B@ý3?="/œ+Õ?SŨšTb?CÀ㬔-?ïÙ´G•?s>'>àÖ9?Fià`š9`?[mM£[k4?pX¸ßÍ3?mHÖQ¦X?ïŒqЧͺ?'I\"O]®?rK߈Áþ?yt2QÂݎ?ƒ½üñöÜz?z–ºìVÖ?ïR-ÌH?omI$þ9q?\Š6èõ¤?D÷xÊ	<?"ñ¿†¤Z¤?mV‰©õM?ïæq7C?\±Ìà}·›?R?1?KŒïVâ/'?`'»h>ª?Sa~š™¯£?yHR?"CSþ	#Î?\e³|‹?vàÎ?н?Š»"5ô¥ü?Cc{&F?ïE‡¨DF?Š]†VZ?~؆ˆª'ï?'PgZ(?1Ҝ*Ô¦?'AÇtº¼?îK˓øÖý?ˆOý9V{?pHa¬æýù?`ŠmՏÝ?©::‹«p?‡1~<šAGN4FGL J2318.2+1915?ï9z$‰LDÀC4t}€^_À9²Áo¡x‹À<Íê>y@ËO¤@I´˜c9?¶Ì—Þ-G?|¿ûûZ÷?Å'T,þ@,½£9+¿à\VbbJοæ–{(,¿é0¸.°¿àÆးø¿îE·Ï冿ïü;ºÁ1ŽAGNbcu3FGL J2318.6+1912TXS 2315+189?ïø8‹aÈr?@òŒi¾¤ ?.	¿x•N?!F'ɗ4?G›aŸ{é_?<®®-¨Õì?ïãßìöI.?}xÅ\j¸?2­—2x+—?CÊo‰Åë?iÊ`+<Š?|ÌP6}À?ïÀž-}Í?q
vÞH=8?Zߣ(RÃ?dӘsåæ?xùfÀ?jýäÜúi?ïñ6"Á?@#g8?7"µcné¡?"V½C~?W®Î!E%ø?;äãX ?ïó›±T~æ?K&w<oT?:‹ù
s
?1}iN3W¹?R%Ÿ í
…?FëIå5ç¼?ï²è†LñÜ?YN$ü?K;¸O%ã?uÞ%ï6±Ó?'"ï{å?‡…ÆM¤?VûÔ?}úäå(Ø?cÔØÞoŒ?jµH£g5µ?†ª&;?z^0ºðo×?ïÛ
VÍ
²?^]lnÌ'?R!CÚ½Ö±?F	хG±@?kâI²êæ?Wë¡{ç-AGN4FGL J2319.1-4207¿îǪÜë†ÀP|+IºÀ:uú=H_ëÀ<•æÉÎ@,ùÏdVÂ@.Øà×EÍ?¹oÛÛ£
¿ŠŽÈvÉ?Ñ«Dœ'x?ý6"y þ'?è÷Z_G
[¿ãmü\ÝP©¿à'Æ-Vпà…à19¿âW°ö­pç¿Ûâ H£ÞAGNbll3FGL J2319.2-4207PKS 2316-423?ïÌÇ%ea¦?€EØ?K(<Èܧ¼?O¿XíÖé?v7e›0	Â?|Kx>N?︫Ïôkð?}_Œ¢Ñ)?UF¸ßüª?X&›R/èp?~Xiççè­?xÅIKԎë?ï{ûÊðð?v r2Äź?aÉ{oÎù?X²'áYüÀ?ŒŽÌi®"?t³ÅÓS
©?ï)[exÍ?u[Œ¹1"?mÀ˓èç?Q³'Œ9?˜â»"_¹??tO›–mn?率âéCÑ?v£]ð" À?[£—®	Θ?Mi%ÕjT?ƒ#C:?tÕkƒèø?ïN@ÝÀºñ?"õ®ºµj}?bÁ†Œ
w\?l?úNX¸?"ß³v'íÿ?"†µbä+?ï;§SŸ?'$׬*?nÇr:õ?d*kûæ?˜|¿•Âú…?Ù<®Åš?íŽH@I?'_~&á?'Ý'4#æ?n½Šwƒ=?±2¸<i_?'¾=Lm•%AGN4FGL J2319.6-0456?Ú4ssúÀMkøüÖÔÀ:ü8ç¨fÀ<‰á<ÆYì@ '¦un?ú ˜ u?лR;Œ/?΅xdë'
?ÿ•S¹»@þ€G7w¿ï嵜.ŸP?ëýQÏÖl‰?•	i¤ù
¿Ð:n%wˆÎ¿áj3°0´Ô¿áI€|'!ÖAGNbcuNVSS J231929-045640?ïÛbã`HP?bëvm÷?>ÔNbŒ?0À1'?paI‹*;K?a¦NN½¶X?ïÜ3HƇ'?pÐÛ1¹ëZ?@Ä.áNGÁ?GÂ^7õÔ`?o›«¿!m­?mËJêՎw?ïuƒ>¿j?|ÁO¿ßÇ?cG(ÔÄ?c·ÞiÈ?Í~Hfhm?z͊×pÔþ?ï)"ô¤ŠÂ?rò9Ǎ¤ï?_֪̌«—?BÎe«[º?˜Ò˜—$Å?rKúÍ	·P?ï¼÷׉á?mz'!5¾?OÖ¥]|;?A} b§?}‰?˜•j?k®Î&ąñ?ï.óÍ?‰:#COUÁ?Sç5'¢y?`0¤cPJ.?‰·\—}G?‡ë''w˜?ï'ܝ
¤?†'Ò–j"?i,ÕhU=š?d5&9dú?˜è)¹P²å?…ì]Çí{?îEB*?‹ƒl#d•?fÞ3òØ?WA*—Ð?ªBÐ=¨S²?ŠÚˆ§á)AGN4FGL J2319.7+1609?سá[-ÀDªiƒQX¸À;/=÷²S¥À<¡ßòC~Û@ ¯´õj¥»?ùgk´"«?Òãk¿ì""?Ԕ–e¿ã@Á}ä1@düsÙk—¿ïþ›vóQ?ïòh!ýU׿垴‹g\¿¯>'iÈ¿á×U¼Ê÷
¿ïó¬ÐDÑAGNbllRX J2319.6+1611?ïЇ£31—?hQí®ÿ½Q?GÏëð¬Óß?:$6]…Ë?tÂ0Ð!'?fŠ±Úc$q?ïª_}F°F?~ÛzÅÝ)?X¹Ln˜æù?[ÍøJhª?'P÷&°‹?yæN
·2?ïLß\F}?"òX:gO?i°[(wõ?e†Áòöy'?"F.­¸`?ƒi5À?î¡ó"¼?å˜
'?w†ý`Ÿ?`ø­ô@v?¢ïïï?'-?ÓYlÏc?ï·zèÔjP?pV®Ùÿµ?U)ÝYAü®?H§:‰ß?~øHiTÈ?n°Õs°?îå­Î|FÅ?`p`ÃÃ?nœj'HzÞ?zfªgϟ?Ÿv¸æ]d?™Og
®¨ð?îÜ°Æ 4?'¤j<¨O?o¾}®Ý?l€FKeÇl? C—·ÆË?ÃstÅ­?ìñÏüÜ×?˜J§Ÿêâ$?…4®4:­?x¶ò¡ÆÚ]?µÊî;·… ?—,e‹5'ãAGN4FGL J2320.8-0823?æë7';ÒÀNőÙýÀ:Ÿ>ÔI™À<Q˜hA1ù@j×9bL@2Á¾{Ñ2?Û÷Ü°ožô?Ú+ഐ@@¹áåéÔ@	P§d?ïûU@¤4þ¿ä©ÅÌ'‹_¿é€¾×@Ä¿ë‡Làƒbö¿ïõN`¶#=¿ïÿ%D]'#AGNfsrqPKS 2318-087?ï£$± …?~ƺ˜øI?XC*1aãÔ?S¼Kmøe?".nfÑÜ?{úɯhè<?ïŸ *±ž7?…G‡5æW=?ed6ŸEu?o†eö¤Ä?'Þ皙ü?S¥Èì¸c?îþÚ‹ÚÈ?H§¶(JÁ?'èk3^¸?ºìÉWz?–¹¯æ?‰o­©7û?ï"ñB‰#?sM?}N˜?rψ?´^?\°[ú˜2?—)
÷V¼?q@ƒéZ'c?ïnmóðÊz?ØȚ ñ?f
Ø9Î<?d‹øy«‡?ŽáçóXx?‹K`©ø‡G?ïháÑýÊ?¡Š@Ðɔ[?|¡ºqKž?ÖuúZP?˜ªu@>Ñ?™LßœX?î'Ñv?–¦Úâɕ3?ƒÊðóÞ©?'bƒÕýk?¡ð3ëP+Î?'ñd`–ˆ?íä¶_;é?'²úqS\ý?{˜*«'¦ô?vv
£®¨?®A"º€§­?'Ñ{Ú­:AGN4FGL J2321.0-6308?»i—¸ÛÖÀIŠiƒQX¸À;[ìëPFÀ<îUsÏÛu@ ;òÈ	­?ýDÌh"ÿ	?ÉX°›>?À¤ÿ§j"?ó홖>›F@nr
—~?è¿Wߣ¿éì¶wò?³
|%js¿áMÚ~f7l¿â>™˜ÂÚ¿âw®aÐ*AGNbll2MASS J23203986-6309181?ïèœÅ"?Q?Vª—RHv?1¢u¤'Ði?#V¾/v-?e.ëëíï?TÚCãÌo?ï©â䳕¼?€P=:Œ-¡?Zƒéü¬è?_d·í?'DÖRÃU…?{z>Ì?ï{¹èf?zŸŸ±xjð?ZŸM/q?VOmª–)Â?½Ý=R¨?x¿ÿIJÆ~?ïX'{Ö÷.?na'=gؗ?_'e{ºu"?D8ڗ@Uš?'öŠ2ëÖ?mÙ¾'¾Ì?ïÆÈ>¦6"?mÝñwýï?HoG+îØ?=
¢QŽŠ5?y÷ђ—7?kŽX+
íx?ï7 ¬?–À)@å$<?byÛ~b{á?m²œä>Ú?–Í´–Y¥?•É«9'
'?ï#£Ž!Ü?….qnZ»?a?'ÁÕú%?\Nó¼#?™c›äU2??"ˆ@»7ø5?î$¬M·?‹—ȲV–õ?p[}M·Z?biÙU äÁ?«±´²\†?‹&È!ß|<AGN4FGL J2321.4+5111¿ÞêÅ
ï5À"hæŽ>ò"À:7{~% À<H¯¤Ùš@þI'¼1Ÿ@SüC²Ý7?¹2·ÖEœ?ha[¿¸J?±ww°»Ÿ(@dš´KÍ?âmy_èGý¿®e!0Á¿éõP¯Dü‰¿ÕXÅÉ£M¿Ñ¿

Áû¿í)\_§ZwAGNbcu3FGL J2321.3+5113NVSS J232127+511117?ì'XBiå?±.ñe¸Šƒ?mF­wÀ?`'£B§ø?»Ë´ÒbÁ?°÷LªÌŸ?íÙ÷-Q$"?±ç©À—Û
?Gx«»l5?ZTðª&w?±V•®ñ?±´××z¢I?î9™¦|"ˆ?–™N0(?qd¼V?j¶è<s?ªF‹äy?–ýå‰â5?ïªÄÓë5?a/t`ÉÊ1?Sߑ¼­Ä?8ÅM( Ñ?'þ£î<ú?`‹Š_c?è˜æo|ï?À¤QŒX•?9Þ	>yÚ?s9ñ6Ó?Ì¢—S2ô?Àc§
V¬E?êÊ¿4†?£µs·)D?Se3¡p:>?j"QïSë?Ǧ
œ¢HÑ?ϲҝ?ëò‰·#m?£—v"Íސ?VW¼à´¡?yJèt³²%?¾Døº]ÖÂ?¢Ãjîo÷?ï	 uÉäC?~M¡_<ü¸?p54õÀ?^"BÏ«Ìé?šÎ¤gÊ«?|eånЉmAGN4FGL J2321.5-1619?æ?¶ŠÑDÀP¢øa¦
EÀ:2íÈÅ×À<PšíV°@ R""Fô[?û\ãJ½"t?¿']è¾oè?¸½ßÉÿ'ó?ü`q$/Š1@Òú›½
b?ïÆ•Q5}¿æŸCâ­ß¢¿ÙoD]¿ÇM»à~í¿ç€N9Hö꿧Û7TAGNbll3FGL J2321.6-1619NVSS J232137-161935?ïøL?HÀ8?;	€¥!ë"?"Âí>½õ?†¥+?K¼‹X¨Î¼?9z¦3Ð}?ïètˆ	›­?kÈDäHÜî?2× †ßâç?Ag°…ôÂ#?e0"¨_Kg?hÆþ&ªš?ï¶Û»Êhf?rTjü¨P¤?Q»v	-è|?TT´¹ƒ8?€¢<qõ?oøxÃ$sM?ï¤ÂV$C?aƒHZìv?GêŸ2³"}?/Fε7yÁ?…PÀ‹µX?a|ŠÝ³?ïô,–ЫB?Döæã?++½Ç?Ikõ—ªU?TAq)ð$?C%-qâJT?ﶃò_ÐÂ?ƒ3S´?H4vZB?[TÃõ
u?€ÛÃ[D)g?©ö"éK?ï…ñ:º?}aøÿ>é½?Zù7OQÀË?W¨÷´ò°u?‹$uÃ5%O?{õh]E°*?ïvlÌd¦?|õuA†lE?[¬š»Ì]?J©ì]R|o?›–h»
Š?|E¢âÂ|AGN4FGL J2321.7-6438¿î€~®0ÕÀHì° Ä›¦À9µKÀ<p¨O?t@Šû"@ÈqGÐ?­;Ì´Îÿ,?G•๗%?'Õb垼@»¨pL\¿àp¦€Ýµþ¿ÞŒ'àl絿â>=Áç¿á»i˜JA¿å(ǟfb¿» ×»é$ÇAGNbll3FGL J2321.2-6439PMN J2321-6438?ïõϒmf?c¦ÂÈÎ?#j#£)"Ï?-k@'áx)?Qó—LÇ]¿?b Á¬‹Kg?ï_‰Ü?d™Áúº/Œ?&ÅafJ ©?;XÄ×?BØ?]àh?Ú	?bsñƒ)Y"?ï ø2"´W?~¦Ž4ëÌ?QÖ(®†xó?WєcK?…‡.^Âk?}ÒX	#è¯?ïüîkê!? ‡ICs{>÷"YìÈI>âÀY8ÄÊ?7\SqÚ©?ët"£^{?ïô( äÔ?aÌ%ŸW6Þ?*úìlû•?1gǜa~ä?TP}K#L³?_¦
{ìE?ïÌï")<\?70'y?1Y÷#›%§?HP­?xrž{&L%?€›âça©?ïW+¼O?‰Ö")zé#?\ÒZÁœ¶è?c¯
ñ?"RTßËð?ˆ÷(@n?ïøqf/ñ?Acª"Äë?
4+*(,m?)tÞńZ?M¶øÀ<»Þ?@Ü瘔|îAGN4FGL J2321.9+3204?ÙÜ€xá=À;ö<1ßvÀ87[‹ABÀ;‡³äžzª@Øם
gb@Hƒ&Ž? 'FJƒ?¿ò.±fS@ý"$½@Y0Eíõç¿£G>ÞF·¿Ýû†ß؝¿ãJ|àü.º¿ã¬fZ§ìC¿é袠ÿ>¿ëB&¶M.‡AGNfsrq3FGL J2321.9+3204B2 2319+31?ïµþäù6?r'½uÍ|Â?]»ž ˜R?YxéØm?}Þýnó?nÖ¼=G.?ïÙ]¤ÿ[ô?r!œ¼rO?AÕqiÐzŽ?O"a½XD%?qat»?p)2ËN³o?OÈa¦?‡÷"*?z€>Òï=Ê?ƒ…mú"1?z¾™^ÝoU?z'
S®Y?ïßiÕâ?U˜Z±|¼K?D/3ô»x?1÷2—?k‹ô5›?Rù¬aAîH?ïkÉٗ$c?ƒƒ!ï$KË?q¬gñŽH?p·HŠÂ?Œ7‰c~p?~QŸDªZ+?ï–>P¦>K?Š'®g(z•?a'yO?wGÇm©?†,G_#ÌÅ?…ö!V}?e?ï0ýòÅÀû?–ÿÔ!"þæ?‹À短ù?'}†ñÿÀ?‡ÿ›½Fƒ-?‡]^åD'?ï­r®/?qÍ
4R	f?XQ'ï±SJ?I:ÇDo°}?µG×â?pz×tŒAGN4FGL J2321.9+2734?å5Ë	À?;Y5ü;OÀ9"¸ÜU
À<4›ök+È@w>ÿ¥@¦pâÁ*Ø?³¤ëÝ3L^?¶Y"€a'@³â…›µÔ@ܰљ4?ïåѶ@™M¿Þ¡NÄ´$Š¿äœ<I	^¿ÜmÍ"ˆ8¿è˜¢ô¿åt¦FPFAGNfsrq3FGL J2321.9+27324C +27.50?ï»ÿw³?kGMõñ?Qž¥@øå?BR®Z­¤C?}˜Ž¨¸a?i5e~ó5?ï:)àµH2?"
+¼ë?vƒsN§?}cÍ)rûÚ?"6£ßûÜ?Gƒ–/ÔD?ïD&\Nú(?ƒ¹;Œ'&?q÷ÊYY}j?rÞÆã{?'ýAÚvö°?~γ©P ö?î€/¶ãÄ?z®7ª¥­?'%ó^ÐӔ?m0³÷rΎ?ÔÃ%ò?rä35T}2?ï^Üðõ?'Üiñâæ'?k~±)ŽßÎ?`G–ïԏh?´¦»@2u?€ùÔid¢¶?í¾Ž	‡W?®^ÿê±d?ÛÍñú´?—òz:Áx?¬ +íºEE?¦¥Sƒ'"?î1S
OJ|?˜§Ý¶]é?‰Qà«"™b?Š¯¹B`µ"?¦–W,Óé?'§–KJE?ìZJ {ú¼?"œ%‡po?¦Œè@§­?‡ú_¡u?±ç¤ˆmÉÈ?‹Îêq=þëAGN4FGL J2322.1+4440?Œ}ìÀ.·¤ƒ§ À:©È"h¯íÀ<\§D}"@Çs){r@'ä´J?Ë}õ#XÐ?ÉÓQáŸÜ@]týØÞS@þ#ØÍ6)?ín«äõ¸~¿ÙpfÅ[ê7¿æåà/Ò¿ßnwa¶Sd¿ìðZÛî¨À¿ïõ_¯"AGNfsrq3FGL J2321.6+4438B3 2319+444?ï6¬DÕ%?ˆ:ëfÕqî?t$8üW®?gyü¢%Ïà?"!`×Cw?"P®ÏKƒ?ï^qœU?'ŒûM)-À?taX¹ðF8?tíj$Ù¢¢?Ž3ßט?JKõï'b?îÁ³ˆ?'Û"2š«?ƒÉäÀ{§?}֘¨*õƒ?ä«}×":?…æ •R¶?îi–Ç'5?~¥n‰'Šù?"
.@ùþ?là‰^W?¥2ÏsæĪ?x€èˆ.?íìC;Í? "V|¾‹?‹K™^lø?~Q§‰éš°?ªhé" "?˜èÙw¥r?î;÷ï÷Z?©Ï:ÿ ?Š ËÛéD?æµT€ÍÕ?¥Æ}ˆ"
?§O‡zþ»í?í'³¥£,? "å/:â?"BvÙ6xÉ?Œp#×à!?­M™Ušôà?šB¦g›?ëBïRÖ,?–ç£fÍ?¥
õãà?‡Î.3µˆ9?»Zÿë]0³?'ï& ͖QAGN4FGL J2322.6-0735¿ëThÌaîÀN¤gbèÑÀ:|©B"	À<Vhiuå_@+ëÞ
ò@bå€!ùO?Ä­Îq?²½)썇h?ìrAÁ@|@|e´å¥a?ïÿT>Eµí¿Ö7@¿åº#ý¶#¾¿äc4^ÁV¿æ6_½Õ¹¿ïÿÀ_V&ÓAGNbcuPMN J2322-0736?ïêý]t‹~?SF‰ë"o?')Ûs¯™¶?`"éõ?c±sâœ?RÈô.rOš?ïê'úm3?eD-/ÿ?,´]·—Ð?:ĕ45O?c£¨Uez?c–I¥—|?{*‡'?'Eo5ðåI?]Ó±$ö
Ÿ?c…x§y?Š+…¯Á?Z'¨ªÊÂ?ï×ý_E–?R1ãz×Ã;?6lÁË
f‡?.¡Yï‡?rš"b¿)®?Q¶œóŒóM?ïÔÉ|Ïù?j>ÜôŠ"?7T
1•5?,)i7B"?t&©?ia¡3 "?ïÈIÜÜ©(?~čûa"ð??‡xA«¬?PŸ°t1?yâ¡#"mT?|x¨Â³A¬?ï1¥f×Oˆ?‹ž"ezº?gz$~ýpŠ?g±Ã`*JÌ?–ܐ÷?Š'ël£€ô?L˜Vp?sâ{ñ¤.?NrPWÑ?<²N™—-"?‹øGх+>?s€7ˀÂAGN4FGL J2322.7+3436¿çoAL·¤ÙÀ8Ê!§´ÝÀ:ñ
™¶öÀ<T_°i¿·@ 1͒ð] @'5>¦?²Ûù ÜÚ¿¨›ˆ²¼U?öôÖ¡aä÷@BY@ãö¿èŸÁ¦Óê¿ÝçK~-­b¿å§Éþ;YÈ¿Ýu=äçöŸ¿ØºËã˜Á-¿ÔÔúc
AGNbll3FGL J2322.5+3436TXS 2320+343?ï¶x?+äà?tM׏£•?Kê‡Íï¿)?=¸YÓÊ$ò?€£GÀxsŒ?s ¶†%?ïÂÝú`r ?zÕ'€¸Z?I"|큫Ö?Q°"¢p?{^s(šÁ ?xl¨'/?ïi‡ÀÔ ?}!‹£0?`ÇeAÝJ?R/Ä®4¸?¶$–l¦b?|
·^¾‹È?ïD†à&?rÝ4…º?a*A‹??D ãƒÈ?•XW©?qæ\°zÊ?ïLÐï'j?ˆö-‰2?bŸ^$܁î?T;Óhcëß?"öDêç?‡gq"œùƒ?ïE'áèµ-?"–mÙç?^=i­A¼?j1/Î%ô¦?•yäglM?'€šan²?îÈö™í?ä'È?mY
SJãÓ?e&hhñ?¡›8ûµs?ŽV4	ßâ/?íÁˆãWÂ?'´zç?{·dù.u£?i>Ϊp?°8
g»ˆÔ?¬£Ÿro¶AGN4FGL J2322.8-4916¿™Ë˜š@3ÀO´á¼©À9ʾšÚâ9À<
¦{)l
@‹]"•{}?ùÉ¥¶Žj?¹­®#"Y¿?Æj Û'G@ܸŮËZ@ã¸>Jh"¿ïý2%9þ?ïÿ"D¾Â¿Ô¹`¿'F¿Ñbf¼ønf¿åǞ?È¿×pŸ$rüAGNbll3FGL J2322.9-4917SUMSS J232254-491629?ïôù"ì?HFy!`øó?G¬ëÑöm?>·y˜?H/0`qÊ?=Ykq*l`?ïÞUá3E?r
}?šlw?Dº¸þ"Äç?Q8{ÜI€?l{p·>Å_?nB6g
r??ïf;…‰Ž¬?‹÷A*(?wÏŠ#?€R
tÙ?Š‰'óö?…Û¸{p´?ïàù³o?x+yG
Ü?díKElQ}?JÏFÕ[?™†7Ya÷?vÈê=½g?ï昋gÊ?[w3L?[" zìªÃ?Q+iwšn?WK\ävPƒ?PEiÒT++?ï™L{Èg&?""29N?]pè&ž?p
α"µ?…þÄMΟ?‹
»'pc?îú>'yÿ9?'ôvÚ"{?"pq"YI6?‡IÀ‰	¸í?–õ	«8?IìÞ?c?î>äF2‹»?3"Íš¶?q©òØÔ/Ö?`cÂîä¼
?©Ü}AdÈX?ŽZõ˜=¼AGN4FGL J2323.5-0317¿æjFDTe)ÀMO½­uÀ7勾åƒ}À;~^ÛWª@¿ÈVÆ`L@HAíá?šo7àü®?¸''	"83@¡e}'%@Éï"µ¿ÑTù²W¿Þ¸ô¾-w²¿ä¡:B-ƒ¿äxfÿš6¿éÏ¡þÂé¿çÞ7u¦AGNfsrq3FGL J2323.5-0315PKS 2320-035?ï¸×+ÂÈß?Š­x¶(?Q¤óiï‡ã?HÞ9ãJ‡?+-3¡Žw?‰ëþö}É?ïΏY¯Ÿ?€²ò9%?LDèrS?a^!ýåvL?u/¶Fž¸?~«¬¸i?ï­ñâÝU?'ZŒÆP÷‰?k¢£€
±?x ¤ÓCs?{5½
?yú÷_vøÐ?ïå
wÁòB?Qd4ö•gÃ?:¥6ÄõBÉ?*–?g á$R¸?OÊ­	yU ?ï~^[;KA?…Ò5F§¼ï?R°9Š
"€?N@vÉ-?ŽbD?…"Ž''ä?ï—³ã"1?Ì׋Lã?Z
}B&:Y?qk'Œ¨Ï?†ù#gÅ(l?Œ?5^¬iÈ?ï‡åJ$Ää?‹¬²Œ?úþ?s"¬µÈ©È?€cñyyór?"DWBh?"Ec:ý¡ë?ïÀ4ÎÓ?k®jɐïß?N%‡×¦?A­JÚ<è?|-!QÛ~9?i÷Sáú•AGN4FGL J2323.6-0617?¸ÚÚÈâ'?ÀNBàP7PÀ9õ¸Ú§€ãÀ<àŽµ:@‡|"P.—@é=¿Íá?»ðN²º¢?ÇR¿€#@	ÞRù¢í@׵̀?íri^¾Q_¿ÚˆüvÄ¿ä˜Pž¨ø¿èˆ4ýbÁÁ¿ét÷Ãñ[ø¿ïy
]QïAGNfsrqTXS 2321-065?ïÜO=Í7x?a 4:\®À?Wéµ{ †?N5=|Ž:–?g»çhÙ¯?YÕeÆ°'?ïìv0ˆ?i_w8¸"Ÿ?1ÉÄ5\fn?Jq¥> •S?aP—rÑòd?dîÀš­÷?ïŽ}á·?|Eì=icº?o™'"ó»?n¤Gž€X]?"'üey~?v~ð1<P?ïèûö2?F7¢yš—ª?-
Øm4Kå?dq"ï­Š?e4F=Üñf?E$«,u–^?ïÀÿiñÐ?pVß'ÊÍ?eÍ_
ÓËË?^Í%Hu ?u
PªÐ>@?g"©§ö€?ïËÔ_z±?\ÂÎô%Ë?<᧗#$?QƒÜm§—?xGÛÀsâ?€'`.tJÀ?ïƪ–8ˆ?TJ†Á7´?ƒ7Ÿ±½# ?ƒ±n²Á?"KZÏâßf?"øq˜5Ñ?ïüËÖ`R?eèÎß®?Bñ¯ìï?2+^D>éô?{à›ØVwj?e	FNAGN4FGL J2323.8+4210?瀁ÅùÊÀ1ÍýÞ½À8«€U¾À;"wï$æi@L{)#Ù?ütwéR?¥ÌÁ¶2?±v¡G
Ë@.xžwNì@
Nv/²¿Ù#¸ÁÒó­¿Ò¢Ÿý‹Üm¿àJg,_œ¿Ö(ÑE'пÜzptb¿âÓ¿°.±AGNbll3FGL J2323.9+42111ES 2321+419?ï¤ÀÁ?¶IßíÇá?2*ã	áÑ?@Z±Ý~Ù?†>£n<Ô?¶SڟR©?ïà²ýe=i?pâ·åEÿ¾?BiåÝiN?M?:±Ë?j²žV‰?n/G=óªÙ?ï¢î̞K'?d«ò}ޘ?XdhíÎ?b/,­xï¹?"7¿¾€0¢?€.'\µ?ï!a·´?ygyäƒ?dþÂÀ:âd?E=.´{('?šüWJ/G?x-—Ÿ†Õ?ïÄÌíGÛP?ŠU6f?Dy-P¸?A·Qfƕ?{š0,j…?‰²–R­Åø?Þ]K"?o"ê0«‡?ct/2æ#?ˆðñঠ?'?<˜BÁ?"ÿǑr°V?ïlDpê›6?Xɂ°íö?bƒø©9Á¸?p0ˆÚ?&ò˧?ŠðGµ1Œ?îYìÒÉ?x¯sˆ~b?t¶&&67?]Ê°X?«ƒœkÖÉÃ?Ž½ªƒW…AGN4FGL J2324.7-4041¿¸:Cq|–•ÀPå6&,ºÀ9+þ¤¶-NÀ;¼çºŽÜ§@Øc1R³V?ùùÆ_ËA²?³1`n™€?µ©¸J´¯@å:a$Þ@H€ú?ÁʹÍÇè¿Óf$a´%¿Ý±äíU¿ÓryšÑW¿ÙÊûçA˜¿ÖìsԐAGNbll3FGL J2324.7-40401ES 2322-409?ïöó2MkT?@÷yEÕ²?ƒÓA1«?¡êÅ"Þ?P±^÷És?@U[È:%•?ïí!œ¢?gE•""Š?0€ZNØÍ=??rjÚáå?`ÎîBÆמ?d¢¿Œå,?ïPÓµ§Ë?]¿¿AJ­?YQyéQÈ?\#PR?‰›ÌÔÎ\?€˜áG·w?ïf5XsÖß?qNëvä>?@ˁ c'7?%þ¤8Õ(^?'²øâÀ¯&?pÈw¹Y,^?ïí>–W‰™?V½)"Üv€?(Í`7?§^°v{Ö?a9Xìè?UµFè·Ü?ïÁ'-B?£V®ýÌÒ?BqÎÁôø?Uå&¢?|é/£ðP?€\O•I¿?ïn"¹Òbþ?‡&)ñ|?Ó?\m¥¾Âæ?`|c÷uë³?hŽl'd?†Šäe"ÚG?î±ãlBë¯?‡Ä=àtð?OŁï{å?<ñ'ƒLP?¤b³8#<?‡nؼrÀAGN4FGL J2324.7+0801?ßµá聣ÀH†`˜À9'‹©ìÍôÀ<$_iòâá@[(+îz@"­ÿ'+¿?´¾¿iŒá?§k,Á "–?ñY×\rǞ@	Yh&/¿äƍm;¿Þ4ÓpsÛ¿äßd¥Ï2¿Ýx`«¿æ¤"…|+¿æòø°€eìAGNbll3FGL J2324.7+0801PMN J2324+0801?ïðr:§h?T.ŽÔ[Æ×?0TF
yØ?"Í£‡'.¹?[ÛF&'·?Rª†/;MO?ïÞÝDƒ•?q|'°§?>ÈÜÎa§?KÑx>1?mI :Eø?n2»sÈ÷?ï¾TÈóé
?o+$MC;?RØ­}<›Ü?F›ßIðó?|p=i¿Ð?nJ*EKØ&?ï¯fNWjº?`]ÓtK¡R?[Žƒƒà!L??6Þ: }?€´œ	ÏwM?\øÝϏ?ïà–‹Ð¶Å?cÿ3'K~?A)^mIo?4œ©\°?k0òç?bD=°ÞYe?y"Òœ?ˆz¹RÉ/ò?KÌËô'?ZP}_—?ˆ bEüV?†ìz§á½?ìӎ™?|\Ô¬?[ª1Fêå-?QL©Ï½?ˆfþ®õ‹?{0ãÚPà?ï<R€í?|%B¨pÊâ?qÕýÜ»?]i'õù\q?">p&yT?x\ý?‡¬AGN4FGL J2325.2-2010¿ê&z²<—zÀQF¿]xÀ:ú"=_ À<¬˜ÜÛ7Ê@ Q$"‰åG@Ûþ +ïr?¾ôöŒŽÄ)¿´C?šÊœ?ó$5æ€Ó@"†ÔE,?î:ߎñ¿åM¤c!7ˆ¿çti>2пÕMW—Õt¿Ö(`¼ƒS‡¿áæ7¢-¼ÒAGNbcuNVSS J232520-201213?ïÏVTþè†?‰¾­†­ì?A"ŽI˜X?3'b€ñ1§?v3bÌᗠ?‰¤®™²£i?ïÊÐU9å¡?zúl#?Mp"Sjô]?V
çÓûø"?véÃn¶?vÌS­2œð?ïj>et¶?ƒpÏ·‡j?[. d"Ž%?d¸,!g1?'QFÆBW?'îMÀÈ­?ï¡Pù?i_AÓ¸?F6±½•V?0]ݱ‡ù'?†ZíڽR?iKðëG?°Îÿ?ƒ0ïÖ£ûq?T¡˜€'Î?G¤!©ÆÚ?ˆÑ¿Âü~?'<*‡ûÒî?ï'*J4	P?Œ´O»D³:?T>bV+nº?f¤ý,l?ˆí¡ù.O?ŠYWwD¶ç?î×}g'?_ÞùÑ?bˆZr‹d'?e¢³zD'?¡fb†C6È?«–"+íE?î–óÙ'›?Ž/é6A?d_ö"ªx?X[ä²
°?¥JÏ>
¤%?Ž‡T­AGN4FGL J2325.2+3957?Ðj'7ÛÂÀ3ûªy»­ÁÀ9	Ô¿	•«À;ßʯ¼Î@^(ÿI!?ÿãiÇCöÐ?¨É&O"?½–­@Zöƒ{á@GS&m§ù?ï)KRä©¿½§A"	?D¿âáÝ Y§;¿à—[µ2|¿ä\ËG'	¿ì
³!9AGNbll3FGL J2325.2+3957B3 2322+396?ïåÇ'¤è5?pvÌ"Fo?J[f©úK?MªJ×Å°?c¡þÀ)n@?jbC߃SÌ?ïÓ͝ŠÈy?v'
e¥Ì?Kà7Žš"n?Sj'Þ­&—?r*Ejl¬?tô†V2?ïY3fE˜?ð[(a÷?
PB8
ë?…õ¼øFâ¸?ˆ¨Ö,ÚÅ?"ÿ½~°r?ïYðz  ?l88 ñTÔ?sk¿+zˆW?T_eöfê"?Î¼Séó?fæ!	Íw¯?ïÌ4r3µJ?t "1h?T÷÷vPË?Q£®H*Ñ?t§É$Òv?p쐁Øà¿?ï~¸0Ý®?7ºöŠ?eb-]
'?reäX€.ï?Šùh›¦¸\?ŒÎ¤
G¡?ï*SøÇôÃ?"ïNh)g?"Çk³,m?‰{yîºz"?QËXgk?‹Í¯*8´?îv¹˜›‰?"?^³ÁBh?†OͲJÌt?nÉR
¥ÅK?£sßmP?'šÿAGN4FGL J2325.4-4800¿ïVpšFèÀOž¡ß¹8›À9)ÎPZ‹À< }ðƧ@"E³"@ƒV–åŠ3?­RŒâŽS?£T<ò½?õc£Âˆ@2ÃÈí¿Üƒ€Þ6׃¿ánðx£Ì¿âÿ¾øMڿߜè"éŽú¿âár@<I¿ãY¯åC;AGNbll3FGL J2325.4-4758PKS 2322-482?ïôÅb'ðè?LEò4¢(?&ø¹Ø©(? ̆©€Ã?S–$œ:ì?I'AL2
£?ïì}(!Ì?h@¥?/¢«˜[§ê??pHfLÍ,?aˆÐ,€w?e>Yîo?ï´i?jfA¨ù?TÞ@¾ê=?](…9£*`?yøù0š?d¯÷Ù²º°?ïÏÅÓ¼Þ¡?Yð^_¤[?E£½؞§?.̈́Z}²?uhž'³k²?WgÒ–ÞO?ïêŠócq?X-ðTAšÝ?7d¨µw©?,•?v"}d?bˆ‹40B?U•^%|?ïÆ»*/uÜ?-¶º\Ó??•A6?Que´}?z©¬áì?€½¾•3?=¾c?yÊ2¯"ïy?`ã¬oW¤H?gS'í_?†BôŽ‹2I?u1š¾ôþ2?IŸ†C?x‰&4¾?[ƒ·HðÎy?K°æ5´?Šäv©Øë?võtHµžAGN4FGL J2325.4-3559¿ÃXN[éÇÀQmƒùdoÀ8ö¬Lú"–À<¯Ù`Y@›©ä'@á%Ie¥?¨dË܌ÞJ?Ç:`Nq@jG¾²í@\¥°ÔÏ¿ÓÝåC;>¿ÛêÆ}'s¿ä€!Î\¿ç1¦k94¿íRCÏb©C¿ïÿ¾ÿ"°AGNfsrq3FGL J2325.3-3557CTS 0490?îò!Z7x?¤Ÿjî|n?™\X¹%K?£ÂL¹­C?€¾øpŽ]?wE¤Ëaç?-L
è?—¤'ù™ù?h¾xxQ¢?€J&™æ©>?‡$–¶…û'?'—dt¡?ëp—³˜ý?ª¯âûö §?¹Ð'¨«@?§`Q¸)^?¥U!5(±?œ='À^ã?ï®IL'Ã?fPZInQK?h!‡©g?Sú"ïª#«?|ʖ<_p?_pžaù?í'jèE?±ÿñ}¶X?¯£ƒßÈ?° p–á›u?l‰öKfÕ?‡š€j
Å2?ï%\0¥?¦Iö¶X«¹?xyA¨ m?è2ü#
?—½Óð?¡OžÕ–ë?éêQ~3ô?±N'fπ? äÛò&?­™ñt 0¥?¨×WØ= ?Ÿ'8aÂÔ?ï:;Ä7Ž?€Hü0-=}?{,Õ÷Dý?j'óCïB?'Õ<J­?xË$´EoAGN4FGL J2325.6+1644?åydM	ÀD¹Bá& À:º$?ziSÀ<ƒ»ðÜvŽ@ +Wdë¼ý?þÖ>J¾j3?Ãrµ)B©?«kÿœF·?æRm —d¶@vӉ)‰ç?ïý¢È6¿Éo8&&Z¿àqkè†f·¿âžüå™Lm¿ÁÍ=
!—¿ïþb †ˆEAGNbll3FGL J2325.6+1650NVSS J232538+164641?ï­àŒ@?‡ûg¢U³?GÁŒáÚ?@¹ 1Eåæ?ƒÏåÜïT?‡Î\~b÷?ïӐª1Â?q[¹ÞäI'?@hõç`_©?JÕ0t»Vº?teÑd¹w?o8]¶??ïMš3Çí?†óò¢ì õ?^v֖e4Ë?a±++ˆâ?"eL/åh(?†V/}T€?ï¬ ÔÙ-%?a™é2øh?D썘=¨Ê?0^©øÄ?ƒ©àb¨W?aS[7•5?ï~û">?ƒü'-Xč?[t{|¡ý?Vå	ðÉË?ŒÒ¨{¬?ƒò–ç_?ïˆ_¨´F?"ý•é8?Kö¸cYãP?Y9§lD9©?Œ(ª[BLÕ?ƒ¶ÌùÎþ¢?î¸Ê¤~z?'a"Ðó?d-è¢Á‹?bàGWrM?£0w1³Øê?'þ\U°$?ïWZÚÂ?3B¤ùŸÃ?Z5Ù¬ca?MwZƒŸò?›ñ·"@v?!C°~lAGN4FGL J2325.7+1821¿Ëã¸.'ÀCþwÿuÀ:8(y›ÍQÀ<NÌܽ@Т=­	¹@ÃåZbL%?¶(™Ò#¤¿­w?ö:.?õeU	FП@	Cü ÍU?ïçǟ'UR¿äéŸìD¿è´áMK¿ã›ÔÝ<†™¿ëQ©A­?ڔ‰¤Ùé–AGNbcuMG1 J232550+1822?ïÝMCw?jåÆ3!µÈ?DIœÕ÷Nâ?83ƛ1ê-?mçKH;Ï­?iBîc¶¸Ø?ïÁ—ºúÅâ?u7Û½·?Ldƒys3ú?SMõ\ˆ!?{§'!ËlÓ?r;Õξ?ï¤S°ÅôÛ?~'{mÓ"í?c	?ÂGy?pýLð<IM?'(Ãã+d?xL»øB·*?ïÁtgcš?YIRaž™?T§¬ À&?7K†@ÂW?záÆ`¶?Vîãs'~ß?ï·?×ÜJn?{š'QH_?Vޕ
ü"?P"F`hsÒ?~¨nëèhV?y‹Ë2°%?ï`Õ÷c?ŒÝËU?VÙ#ÄiŸ«?dý{7y)?'wÌ^Jµœ?Š–}R•=?ïks¸ÖÃ?":uã')?f-°N©<?jóߎXr?ž^ë}$?'þA'«E·?ï/ò=
–Z?{h5ýG¨Þ?qÀÏ0ÞÓã?\;™ñôž?•'"‹æ3Ã?x±µ÷H£iAGN4FGL J2326.2+0113¿ÙÄ"%ÀK'ËûµtÀ:ÄfõŸ<À<"Ýao†¡@ºø"æßÈ@ü¸oG¶?¿˜p_õš2¿wåh£M9©?¹¾|§ñK1@bÁ5"âP?ïÌ;ýÝ¿×ø¾BEtÔ¿ÝÇ-ügš¿ëö>¶4ž?s"Âïö"ê¿ÑÓwá¸íAGNbcuSDSS J232625.63+011208.6?ïì²l"
?b¿øÜ%×i?)%F³³E?-›;íÁö?a»?Oìá?aUˆáN-Ç?ïêV¦æðK?gJ>횅y?*Ùø_¾?;·gº§×j?cû¹p5ßk?e/¤^tϓ?ï[*»`>?ˆToÛê}á?^Ԙ¥«.B?kl]RîÈÌ?'­uƒ4´Z?†ï²§rû>?ïó\Ã`¤?=¤ƒZ<?Éá@ëÞ>ò'…&£?Y6÷$Dž?<ÐÈtŽ˜?ïß+¡Ä`m?g†îÝë?:ۓ.@à?5>þ—r"?mxëÓ;"?fOZd‡4ƒ?ïƧ7x"?Ma–{L?:@P÷''?Q|×o|µi?{_=îÛ?}S/¶1?îüJË«?Wí&ßgÚ?gÝ^¿LâT?ríH2•ÉÁ?9=ŽV?ŒùdݹŽ?ïԛÙmw°?aÛÖnxæì?þÚI5˸?Û©ô0ä¾?uJý(‡?aÆE
¬ouAGN4FGL J2326.9-0201?Öã,O"<ãÀLàyåŸ+ªÀ:e^ɹòÕÀ<""ÍŸ@Þ~Ðëj@/FÄàoA?¾ŠÀÏ¿¤«@¹ûÜ?äöÞ¸1µ?þ$qÔ®˜"?ïInÞÛ¿å^m=ðüW¿çº•"<¿éøû^°¿Î)F Mgè¿äC¯'9+AGNrdgPKS 2324-02?ïŽhŠFÚ?€XÇ&ý"<?RwÞ@
.Ê?E1TIS<?Šá´^˜œ?";ñ0D?ïªv̘¨?ƒhŒ]úe?]ÓYOòNj?d£¾`Kbá?§á¸´Y?BÚÉÑL?îäD5Qé?‹ÀŒòd?x n8X"??u'øƒÚ?oP̟v?‰l§1Øv?ïg4"é?vúÎ~"ë?aZ@Tb9§?K.+(«^?›ÑwÚÁ¨?v/<&å†?î†`¨ûûþ?ž‰åe'¸B?m(qgd%ä?c'Ÿä†Ü¹?¥Çn\1·¼?m©»J¥]?ï9n}%'?šéâîÚæ?g܎5ã;Ï?vc×$€?•Öž"ÆŸK?–ùµ|èÍ£?í~ñ"c"?JõËu¡?‹>ànñ±?"¿dbå…?° —XAw©?™ã1·í?íQ$WD­?—Z?9?}6éƒ4P?p©&x9u‹?µêFö^—?–š1ËÓHTAGN4FGL J2327.3+4717¿±*dcŸ9À*h–š
Ø¡À:·V¥ÿªÀ<~¦ã@N´C%?ý÷})÷JO?͈ܲóݳ?͏¸š:Ô<?ýýI‡2ŽÉ@X;¯X¦?ïãĕƦB¿è¨Ö]š9ý¿Û"oH7Œ¿ß}…fÜ­ë¿ä± VL<ï¿ïýB äfœAGNbcuNVSS J232723+471601?ïÀ°ªpÃ?gàh¨›=?M zØ=?;Ö ¢sëR?|ªÓxÄ?fFúq¥?ï/5rÜ,?žðç;ìs?fzäÀ9©?esídmÅ?—Iõ²?bM'%2ê?ïW¸mðŠ?~''œ´$?mˁsâÃ?míUsóï?'O's™h?y«¸nà¢1?î'(×uÙ\?y²îr˜‡¤?ÜlkÒз?[èb$p"?©WoÓwŒ?wæú–HV?ï}(Æâkß?|TõX¼Ä"?aXÊk¦p²?P‰¦©ç?Œ_›©»¼?z¸Ÿ&Ì÷ƒ?íþ¡œ®ˆ$?°ÿæÖÖim?€T~3˜ýø?‰8¯§€•š?¬Ʀýa=?¯oÎQÙ§×?îÏ){pÜ?
¿‰ˆÎr?u
<RÅ?pqDWÊ? m•è[´â?‰îÍߎžÓ?ëE''›&?"þón)ÜÑ?'32WL4d?w½mUE½?ÀÃOlò%?"1ÐT
?ÑAGN4FGL J2327.4+0444?è"
áóƒ#ÀJ"Ðå`BÀ:Øÿ€¾À<f"Xð\@ëâÈÇß@q…Æ}þ?ÃX"ÖĝS¿™."hƒ?ÍêñûÛX+@ùB·Š›?Æ3h7Kñ›¿å.·£oÜ1¿åÀBŠ3ö¿ãdŠž›¿ì4üa'¿ÈK4Ä,ëAGNbcuNVSS J232733+044740?ï«tÕ*ƒ?|iÿ ¦'˜?['dÉú$?QS¬Ýª?°Í§cå?yäsàáým?ïÓØ.C¤?r»PcÆ¾?D ·9Ø:´?LµºT¶€¯?só|ð†²W?p_gí?ï'Ûú3¯§?{òϪʆÞ?cè"Îj?b†_¬«u?ŠNøÉpp?y?e[bs?ïÈ\Wĸ?TìF?D@Ím#?(ž p3[?yIºuê\?S͵£–?ïAs…ç=Å?˜TRÆ?k¢,`F?`æ†:û×7?"]O@£ìÖ?ŒížÐüa"?ï…w—v?ŠÈÂÛ§ô?PXuPŸ	?^<S½Mº?Œ±Sšgçô?ˆÞó˜Ù?ïñÉäîŠ?ˆccU#˜Â?m|qQ9K+?j81‹oŠ©?™R8™êñR?†Rf£NÙj?ï_â?i'-?t[Õù4?[oÙJÂBœ?G<€˜`?'Lº"%.?s+ç@ÝAGN4FGL J2327.5-3259¿ëßƛt)ÀQ½Œ¨À:·pÔ~qöÀ<­æcvÇÝ@ø4O'åJ@3fÿéYË?Ë:Ïç/O?Ȃ;òŸo?ú'(bõ˜ž@¶Œ½¾?ï.Ô>[/|¿ÝzX@ˆÜ2¿çU~¢u¿ée2`=W¿ð?ïÿãåîAGNbcuNVSS J232747-330130?ïÉ»\%ß|?† å}È­®?IHj/=²?D"•"ƒ?wùD¹"@+?…ÑdSjý?ï½¼ H¤"? 
ޔ™)?YÚøÇm
œ?h•På¶?zªñÃ?Çù?y÷¼»åÐP?ï~ªÎRça?€,˸ï+?pvg¬1ÚÂ?vW‰œ?ˆž_?z
Ü0þ´«?ïўþ)Þm?X2»K="¦?Q¶n£$s?9~
±uVº?rÂåPzäq?U€:ð8Y/?ï­*²U?†>@'òYš?TãÅéÚ
?RƒÎ—ÿ?'Úáõ=X?…´€`ô²?ïZ­EÑy
?"䁦1"O?iošÿ¥?z—‹$º‹?'|cæŸÕË?'J²"H÷?ïwF!fF?Œ|ÐëRdu?zŠ°âÿF?|?ö÷(ý?•ït¢Yo?‡A­ÎÚÓ?ïk†¶½ìµ?xʆצï?hCÂx'0q?Yô…ק'?
a¥R®?vOe_׉EAGN4FGL J2327.5+0939¿ïû{j×åÀGü£a™xÀ8¾®×ï?¾À;§:-ù7@w"ìá•@tõÅêZ|?©4'yì€?ÀV:ߤë²@'bØ<l˜@µÌCŽ¿Ê
2îà¿äõÿ 1#¿éŸ¿™£¿è™cé´d ¿í‹Î2JU¿ðAGNfsrq3FGL J2327.7+0941PKS 2325+093?ïŠ{`sñ?¸*TBp"?z‹˜=Hí?§=Ř²O?€Ÿ¾ÚÅV?ªÔ†¾@Z?ïÜ9PÐõH?vn'Ĝ?@:Ïá"Xï?Lˆdê1a?o·û'ªÉ*?t'ŒÆz2Ù?îÜ;
¥¹?–·¶G÷¦Å?'(è7Ø?‡*Þ׺‡=?›h¤^b™¥?"xÀ¨sž€?ïßhþ·_?StI.™YÒ?Fψ°U?2ªÈ?k
á€h9?Qez¦Œã¨?ïZ?›:Gh?¸ñþµën?xGFˆ"ú?ž01é4¡?Luà"v?³ªÈ-:Q´?ï£ÖˆQ6˜?†ˆÿDMŸ·?S'‰ùÇ?kVҐÙF?"¦¡Rpq?"ø…JGÆ?ît"Eµy?šårqGÒ
?í!;DÙ?†	«â(M?¤;ƒ\íöü?™ÜLߑ'?ï—+#Þñ+?vºfL³?eÖèžSVƒ?X‡!
>?"¿|Ý?C‰?sËØ/%b]AGN4FGL J2328.3-4036¿è?ÌQZnÀQ
-à
qÀ8•t/|ÅMÀ;¤BW"dÌ@—);¸'Ù@©Cäõ?£–œÂ¡ƒQ?²½g4@H/yjO)@ǶãV|?Èd¤Yæü#¿ã²úÉ_Z¿å5¥Õ?¿ä%'(]í¿êÅ
á?¦¿áĆ!—ªVAGNfsrq3FGL J2328.4-4034PKS 2325-408?ïÜ-QœÖ?l@7òÅbÖ?D66ülI?9µX)®?nñDìe8Õ?k+¸>òs?ïën:Æ$'?iÑ­_[ɗ?1ñÆØ°Ü?CHXñ8?bSŒnɖ?f^ º':
?ïÿ/~%}?…™»MTŽÑ?ey
BíÀ)?oç³=9³^?‡!ðت,?'á(r'¢<?ïÞÃ
ðãœ?P?|+Ù	?:/ԔgÕ
?"ß–ø¹ì?möú"É'Õ?NÄ=RV?ï¸<ÈïXÏ?u®B»æD?N‡ÀÔOæŽ?CíÁ~kí?€QÀ4‹"?t–¸L7ë?ïÈu®¸²?€–½…?A4µø?è?QòAq&˜L?yž¨RÁ,S?~­ÒˑPÜ?ïNïaˆl?ŽŠ‡Ešn?pf@# 3"?u§}2å?'#Òꮑ?‹§›
û?ï«öN·"L?nᘍâJ?R{¾ìª,Î?DÕä®M Œ?'²ôt1±M?l|ËLVBAGN4FGL J2329.0+0832¿î˜ëme¢áÀHúÁҝÇÀ:X‰ÀßÀ;ú"õëª@	8BÆ¢@¡Ý»1™Ö?Ç/Úx±íx?"%îbYø€?ÆN³×³Z¶@ãçiܹ¿ã6|=鵿êMf»ü¿çµL»šu¿àJæ
²û¿åéázÙºò¿ðAGNfsrqPMN J2329+0834?;,Ò?rÁólšš?Fé¦Ë÷'?8£de†ŸÈ?{؆@ԝ?qó™²c8?ïºä˜yÁ?€¬ê¯Í?M¸–0à4Y?SéVáLØ?~Ö þð7ï?~ž€
²?îËàÄ?'ÊgxÒR1?l{¨3 Y?m¦˜¹§è?¡†Ãý;¼?'ù4+M-'?ïGËêŠÞý?r·Ué¾?N+ù(Ý@?2/—eP
/?–* ÊVÏ?rf¹Ù9F?ïj`fТ"?ŠP°éä­?X͟ÂàÜ?P;b¨Õðb?''.Aº?‰#óòwùƒ?ïT¡ú³‡N?"•qB—½?Y‰È£?Þ.?eŠ)E?"Ó$‡a?"xvæ³?íî+[b?¤;`IÞô¬?ÓD:Ð?zØÛ{ùº?µûZb
Üß?£äC4S?íáw)éC·?'MëdJT?eºG¡ð¤D?Qôm‹*äX?°Fts¦]%?':¥KA@AGN4FGL J2329.2+3755?ÒÐM\î»À6(ö¾7ޔÀ9œÏýÚÀ<ÂVQEm@ LêÇϸ?þ"]"<?±K£—tP_?Œ´íTy u?܉ݤ`r@"UZ$Ž«?ïÉÁ_[ZD¿â	€,A¿ã&pA±{8¿Ôúv=Éå¿Þ›‹Œ;¿Øp¹[UçAGNbll3FGL J2329.2+3754NVSS J232914+375414?ï'ë\Q\?¬e>¹G?RöFå_õB?s¶¥þÆÀ?‰&`d ?©±Æ2£?ïÜ"«¯#w?qÓÁ	'w?=%½^6þ?F³½¬ÝÆ?pNevÐå?p(|¸ò¬.?ïkÞO×Ü?{#ÑìöP½?cك"l´¬?aþÙWQM?	¢Iø?xì ô™?ï7žUÇD?p}fñó@3?hˆx­vŒ?G6¯;Ë+R?•û&Eq˶?nê–Ò¸ö¶?ï}Š‰¨­*?ƒR˜Vž»?[²Ièþ?P/­¢`´?'WUq?Ò–aí
#?ïÅQG46?‡»½fð}k?Qð"p¤ú?`?,z&¥?‰Ð§Xç%R?…Þz×I?cÔ&?¤A=b8?qZSÛ	֌?iF,¿¨/?¢?UPÎ? ýqGzo?îŠïNË?‹"pÏ=Bë?€?ð©økÊ?f,Q[è?«§TÜêëà?‰–äDAGN4FGL J2329.3-4955?àÝð-ŽsÀO'L Â'ÇÀ6×TûÚ×RÀ;A.jv–_@¾5°;@iÂÝ`?‡­ºÚôƒ?»֑ò†@,úuFÓùè@"ùÃǕ€¿›oðAµÆ»¿àe•P^½%¿äâb`Ght¿åšÅ都¿é°
Ÿ@L¡¿ïHG,{ÄAGNFSRQ3FGL J2329.3-4955PKS 2326-502?ïa¶vÒ¢Ø?Ž,yît
–?mËôâ¡ê†?nô*m""'?²ŠS§?‰¿«H8º?ïrÂR‡…?$
ÖvQ"?d6'¤œ?|=€'‰?ŽAÆÎúÝ(?šº¾Ã¤Îå?îJ§D8Oc?¢/ÖÇÍ^˜?£ë©ùçvÂ? ׀ƒ=Ð?§‡-"0?Ù¦0, ?ïïB™
[+?X½Â÷øÔ?@ñÑ*V[?AElÿYR\?YåtÐ?R+È[íi?ïƒÑøŸ}M?€ù˜s.ò?dr)Áÿ9?`£LC¥H?‰î÷–Të?~é֓5)•?ï#ök?¥ã¶ä§5Ä?q·'˘ž?ƒýæIDrn?š-œŠ(§-?¤±w¶ä»Ó?î˕tñÄ~?`Ø¥!?–ŽÀÔoN/?•x×'$ÏF?ý!$ÿ?'´5"
3?ïÒtӑY?qKu¬¤î?RpF'Oÿ?Q?W«T?r)ìëT½?nŽo$i+"AGN4FGL J2329.3-4733¿ëº'´óÃÀPÂÀð À:FM½"4ÞÀ<P!ÀD(N@íb ®ì@ä1æ,c?¿ËÜ!~ã?¥añÆ\Æ?âùåŸ+©Ò@:-1;ŒH?î>rο济¢o¬
¿æ—"[tšÝ¿âh>Õ¿ïÿªÅÝð¿ïü»!©ôAGNfsrq3FGL J2329.9-4734PKS 2326-477?ïóX—µƒ?HãFºè1w??ú£lV?5ò¶µðýƒ?QèÉü7œm?B%û‡Ñ°§?ïßíé}¼?qà}¾"¹3?;P§p÷^?Eª• ~"?l¨¤‰w?pgü†ØZ¢?ﺖ¨3Ìq?v¿·,}ê˜?^÷ÀÔ6?fÿTw'?{3mé†!³?s<RÛ]øó?ïÇn3íËÔ?Z«é"0½?Pó¯t€:7?7«'0»™}?xúmcØ?Y<Õü$îí?ïâP戛×?bm6¡1%?W'
"Kÿ?Té¼%ÆrE?b"-cƒe?WPU¬|™²?ï¬Ôk@"™?‡B ¬Šòi?MטÏ
'ï?dêáÎ"J ?'íkªÕJ…?"q«Ð:Ü?¯ü1"?€%ð΋s#?jà2ė?tj—mÕ_?…TÛö÷Ð?u¤ÉÃkñ´?ïZš7Ï$@?|½ä	Îó?jmfº9`?Y4ÚéuC?'_2›ç/?zª~ˆ
ïAGN4FGL J2329.7+6101?ïÖ.²'[Y¿Ò׳ϝÀ9"å'–pÀ;Â`{jÚi@ ÷u½qe?ÿ9  ?½X¡VÒI¹?±½wg?ó·
1A@9úÄ+éh¿äÛQàG}î¿ÜÑT
H¿ä=Ýܽ¿ÔÐß´0¿äÒ÷S‰¿Þ=Á¬ˆ4AGNbcu3FGL J2329.8+6102NVSS J232938+610113?ïN6ð4¹y?‡ÏêIƃÄ?J– Ê—^ë?B<Ñ҃?•dlñWâ
?‡8úéñ#?à½Á°Ô?ÒHzeª\h?p×@©HzL?"t¦åAk»?ޛ'ÃáŽ?Ò"¼ÄÁæ?îWbæ1ÖD?–y¬Ø…?r4ºq~f?iiÂ3¡?¨C:Q‹r?•7º$«:i?íöH6ה?†)yԊäÔ?|*˜ª½J§?_Ü"R?­,¥ññ?…•'›–Âü?îhûìlq»? rÊ6•?_+»
ÀY?SL屬'>?¨vãa8Õ	?Ÿ¯2¬&n?Ýá{®?Ϥº-§œÖ?tP´~ôf?Ž¿‰QÔ²??áOlíÇ¡È?Ïbó+þ'õ?ìypÉ°?©zž(É?'°S4O{à?z+k?ËfU?½–*<…?¨s(p»Ž?ê«ó5Â.¹? .'X•iõ?"Ží<Z¯?~.[­,ÍÙ?ÂìÁK†³…? F¡ôÙMIXED4FGL J2329.7-2118¿ÔûˆÿdñêÀQ âe+ÔÀ:ÚJcÑaÀ;홭»Ž@Ù"˜€•@¾0O‹Y?ÂÏ
¿¡–¿‹ã­'Ú©H?Èô{§ìÁ@ï¶wö±£?ï²ÌÛæED¿ë棣×e¿Õ§¢Æ¾ì¿éÍÛU%ÌB¿âQ7@¿ïù˜¨)AGNrdgPKS 2327-215?ïwÞ´^tˆ?…'
B®‡Z?[f÷邦h?MkˆWúÚ?Ž›sòÁ#?"Ú"}?ï¸ÈÉ]·?€$-oƵ?Vl°,Û?[M®Ü_ÿ?~µýË?|Í<ñ¼]?í¬7›Í¦g?œ§›DQ"%?Œ°\úbú?…ŸÀ¨Ó.?®:Ú+çÙ?™§KÙ©Fc?îJ‰ˆvÓé?"7ì×·h?lZGˆ "?RèÔÇRô?©—1Ѳ…f?ƒœºãÖe?î‰àˆ¸Ã"?ž~óI:?rÎXù0?g1åˆãòa?¥,pâ›_?Dž¹•Â²?ï?[¨iB?›‰ÈOÁ\¢?iÜo[õJ£?y©šnK)?"Øý )d?—X_`º_J?ë'©‰ª÷?©A½'+Âû?š4ÂÕR,s?'ñƒ8¤Ï?ÀÁð-Ù?¦X}D¤IÌ?댠ҝò?žê~°×p6?€ó/8-:?qßNÿŸau?À¾IÃ(ÅW?ž^\_ZBAGN4FGL J2330.2+7759?çu%'µ@X@/œŸ"…]¢À: ÝU±}À<]pŒZö@ý÷ºa:X@⿐¤(?½¦´4P?¾wðýX°Æ@@Äe?@
~åkT6ä¿ãïa·ªü˜¿æE¿ý±q¿ä•[Fw´¿ã‹B¸â¿è‰ýÅ=6¿ïý«Ç™‡%AGNbcuWN B2329.2+7743?ïÊ5d!"÷?ƒ""© f?^8'y%€?bœî'"S?sW)p0{ˆ?~§ÿJé×K?ïÙCˆÚž?sñbãäé<?JQ¢Þ1',?U+qµ‡[^?p-©äCü¤?oðžœ6y³?ï'O»»?…bëfþ­>?l9ae°ß?wˆ‡òd¨?"­%Ë=A?€"}z×ý?ï½È¯JŸ¥?[k\?ª
¨?`·ÔFI?@]k_GÈ4?xÀ‰J8€?Xô'57Ÿ?ïO$#\?¤°"ñÑù?««gº?Ž¼ë‹ÝKÿ?Š"òX-??µ7u[N?ï)=C¶?ŒK¯;>?]ÿ*Ï­Ãð?ov·bšŠ?ˆ>Ðeסò?‡Öv_Põ?ï8½Â\ ?æ9ïà¯?råúËÑÇ?vü§ù'"?"DéÉDȀ?‹§ê
|Ç?ïBAú²tm?z‡`ÁÇ?vör0s¹)?`C?-Þþ²?'ú$ìz?wœ¦eñ%¼AGN4FGL J2330.3-2332¿ÏQ¥ö/'áÀQÖ"t¼jÀ;t‡'YYÀ<¦ÞãOÆ@gÄW]_@p Ç`?Ò»ûS?¾P[!¹¹?îրÀ.Ù²@d.'Ü¿ïõúÐ7»?î;¼(ßó¿ç"€$þg¿Û#ð_£ÿy¿âý²}–-Ô¿ïÿ?…¦óAGNbcu2MASS J23301617-2336413?ïßîÕ¶*t?ZdäsÆ«?:a.ŒRs+?-v¦Ðå?lÅOœª®?XÞjoñF?ïÕÓPõeó?tÞՍ6œ?Eõƒ™Ó@Â?PsòK"œo?rW§nÏ?qëX&¤h?ŸŒ?q§¸ý Fâ?`]·-bÀ"?KótÝNŽY?‰þP‹/^í?pG'Ä.A?ïpÇæ‰'?iZ֜K©
?bö¿tªç?I‡áö֑Â?V ÿú?gÄô'>և?oO"¼
?o{ãB0"^?O^tx?GÓÈsRÔ?}V,…b¶Ÿ?lӄ8iÁû?ï~3´ãL?ŒåÎ?Wrœ?]›<q'8?fç»æu•X?Œ¿°N´?ŠWéO‹•?ï@ñ·½Æõ?|:ÁgÛ?i 6¢û0?f$Ï4E?"½ÂFJ·ë?|Á¡õ¯O?¤S9—?"^?!
L?p7ìh£?b'ÇSBs?¢_/@¸Á?ƒv6å-ºxAGN4FGL J2330.3-2948?çbõ´ˆÄpÀQÿÐR"JËÀ;Ñx-8GÀ<Áû
Qø@`ŒŠ¸Ö@sgÁLf?»Ío4[\¿·–Õ™úèi?ú#=ó?è›$T"Lç?ïr-^ÝÛé¿â0¶¶àÒ=¿ä/?› '¿Ú©A­Iz¿Ûh¯a,Ü¿å&ÓßÅpAGNbllLEDA 3230048?ï0v›Îä:?·7@Å(Nå?Y(Zì¾Y?'z‹x÷™?˜^¦Þ¹yØ?¶wõ>Œ×?ï[.ŒI>?i½w´o?t—"çš7?ç?‰Á«û?=hªow?˜øßÓ¤R;?î¥Á''?–õïð?tÝ$;?{b™ÁG^•?£ ãæ¤?–azÀÑÆü?íÐûK¡zJ?'tŸÞÇè?TIb²mI?w,/'Ȫ?«›8î§?Žâ%‹»ò?ï%U*±?¢qÕ*D?lå YÝ-?q) X'r?—¸·tnK?¡W	$"?¦À&?µ°¼éÞ^"?"ò4<'
¡?©û,ò×lq?¤®}4ìÃN?­ p¥éåá?4Y?œ;FÞþ×?~úõC"?€˜÷Y$ Õ?«(—h?›¼+§¿^?鍢"=«¡?«jtŠQF?¦"©qT¶N?•Õ̍Yv?Ä@˓"h?ª×2HªþAGN4FGL J2330.5+1102?ÖÝi	%eÀG‰c4'¾ŒÀ9úŸg8ô=À<¯#nš@ZV'©è@õNÂR ?Ç<5»MÉb?Ñ{Pw@ //˜t@
V¡¢Q¤¿Ô	 ØÅ¿çæáËâl¿ç\Á¡ö_¿îWšPx¾X¿ïÿÝÀåãÊ¿ïÿÿ)@k*AGNfsrq3FGL J2330.5+11044C +10.73?ïí÷B¨W^?[/'}Ð?I%oº¯?Gâ~ý"¼?W~´NóKp?TiÒ´qÑô?ï'î; VQ?Œ…2Õ uš?j‰M±b²Ø?w°´Ø­2U?ˆ¢Öèu?…åeÖæ°?î¶7}"s%?—<LMl?€©»S§B?ƒyN•xC? reVä?•˜
()?ïZ‰´|Òl?o´cÑ4?r"Ë·ú†Ý?Sò[Esñ?	–~GˆÊ?kÇáªÑ6«?ïÛ++Ê*¨?me.žr3?SÙd´¯O†?Rdqœ·õ'?jè!ŀ/ï?i¯u>Ós?îŽmGšã
?©¾È"ã?€–°?ª8C?dI-~:?¢ótAÙ?¤ÂRè2Ã?íŠöžàÞÛ?£?˜¾j?)ý ôä?‹Уô©?°dly? ö4Êd?îó§"=›?"7ï›%?Šé'6k${?w2ïsñÙ?§†`ö¨2?‹ -—¥¿AGN4FGL J2330.6-3726?·G¶£WÂæÀQ‡ ù	kºÀ:MµåçPÀ<=æë\@'"Æç@#¥™'¥?³çW'Žž¿±ÑÅÁ&¿?üûÅÃď@6càÐ÷?ïNË	~.¿ç	ÃÞ;µ
¿æu^¡ví¿åw¥[Zš¿ÙUÛ}¿ž¿çŠÄê€;ûAGNbll3FGL J2330.4-3726PKS 2327-376?ïÇm*¶ô?pUדsf‰?I¿wIÜ{?7å"i/áŒ?y{×׌Ø?ox8kñ[ž?ïËLŽÆNP?xx 'Cu ?MÒ6Bqø?T•,9QTæ?vŸqÇþ­?tمë°sk?ï?ˆerS?"Énï-4?ghïŠ>kK?bFBí­ód?•/ñ	m%?ƒ÷'ç.ê?ï´¼ƒ1*ù?ažöµ/v?Z£&s!ÙÆ?C¼¢õ9}õ?~øôÇâ]%?_˜áÌÛ?ï^ÏÅ¿V0?ˆ¢òN_¶(?b˜ÕW"
?RÌW|S»¦?'Òì¤îd?‡½ªªiô±?ïc1-@?"-RQ96?bC‹/Qk?nvéÍUâ?'Qn‡Ó?'×äH*?îY©™c`D?•_Ìí·‡?zFﳘ¨?tjpþB*:?§]Y"&?"_Õz†´?ï	GÚè¢?'Öèz?wÖµ(ÍEò?iŠc €??™É)´lIM?}ýP2%wAGN4FGL J2331.0-2147?åf#µç­úÀQ¾5'Ì÷À90b°Ï@À;ª"Xð\@BÏæ\ÀË@v´âË;Ó?°y5 W?À³³á™b'@c™,ŒP@¹@ÓÚ³¿Û9Î¿Öï=Û,áà¿çñZëÞàÌ¿åW¢žzÿÑ¿ìÛªëÑtÒ¿ïÿyB=KAGNfsrq3FGL J2330.8-2144PMN J2331-2148?ïßVão?a†!ïH_±?YúÑM«%¨?S£ñ[×R?cçˆõèf?W4C3Ez?ïéúK÷?n~
Ԑ¬³?7FZXÚð?Kdלó–Ç?c0i‹©&?ig";>Ÿ?îìiè'"?"‡¶_{zE?†ûáè[×?ˆ$í»¥ª?—jÅ	£±?çÓe!ª»?ïƋdD­?ZT_n?I·á¥c?2B¥uð{?yˆ6ól«È?X–€šýf?ïËÌ1Ïäb?iáÈd	Î6?c†ñKSØ?Yð¼>'ä'?pVniœ©'?bǾs*]Ž?ïÀ´sÀb?'¸¯‹ÄÁ?IQ«o°…?a<J?|{¤K±QÅ?B~ÃhÌ?îpìCà‡?š0êÊãg?ø¿	ª?ï	Z>? óü'¬"?"èæ¤]n¥?ïcåšEˆm?xÜÚ$?cÖÇ6/Èã?Ti.ÆÕ¥ƒ?'sÑdàJ?wRdÆ
AGN4FGL J2331.1-1653?ÝØËG*zÂÀQ3y¦µÀ:êDrØ
À<G¥rë¯ç@¨+i:V=@
˅¤ð?ÔØ[
è'N?³
f
uú®?á"	¶@të¢%p¿ãT°',㎿ºcß½.8¿è7=^ZS^¿ìë»%_5¿ïþ®[È}³?ëUI°ÎjAGNbcuPKS 2328-172?îÈK€({Â?ÅA2²
?:ZŒ¡°Tï?n»)«ÜÒ?£F'æ–`?ÅÊ>…ªW?ïÉá[,Ôþ?z¤K%y«w?PvμYñ?]BŸi¾{?vñžÕûð?u±4€9E!?ïg<O<?'Š†ˆ2"?r…¨ä£Í·?{qÕ&'áŸ?š](ؙè'?Žc5¢?ïÒÂä°]?XYKœ?:ÂM^ët÷?&VôC?tòh»öÓÁ?Vöéi…;©?ï¢Cö"´l?œÇA¢«žÑ?8¼bÀÁõ?Pà´ÔìØ?†©Réww?œRþ"'?ï}܂!ƒ?'bd&¯¼þ?^8:ˆ)î0?o¢¾ÝQ#'?Œö'ɔ? ¡Á‡ÿ?îˆ]Xd‰Ü?–´Ps Å?tÄg/‡?z+¯=Gô?¤ùqé£Þq?•"Žn¢‡ð?ïpjŽòª5?{VE7"ÔW?NÁ­ÅW°ê?CÎ0ZÖÝ<?ü ­'¨l?zórÃöwAGN4FGL J2331.3-1558¿ïº™^`]ŽÀQᛐëÀ:¶ÇǪNÀ<TtûTŸ•@¥¶Ê,@ÐE AY?Ð6̤?®ÆßԈÐ?ÝW¸"Æ©r@
³‰‹"ƒ¿ÊöZlˆ¿ëyJ]¿ßUûļ2¿ê†^¾Ò8G¿á(&à>™™¿ïöÕ´ÒÛAGNfsrq2FGL J2331.8-1607PKS 2329-16?ïôÎSéÞ?EÚ¨fW8—?÷Mš?öÌ!}nŒ?T¢4ÏS‡?DÔÛ!ÙM?ïÛ˜–u?s€n™øyx??JGO­?I>xÕfM?p‰qò?´?q%eO È?ïz®Çý?ƒØƒ¹–6?]ºe)G?h,ö¬@"?¤‡àéÍ)?'ÿÁE¡÷?ïË^;…ÎG?V:Õ@ë?+Ÿ5Ü¿z@?—†Ä²ƒG?ysè¥{Ô?U¯PÀÚÌ¥?ïàÚ|@v?d³Ý-ë:>?+¾öZ¬YÛ?$pjàÕô?m¶67;ê?d<"F"$?ï›vR» ?‹"÷œ¤Óï?OK†¿ Ü?_bKø;»?‡-Æ^_?‰ºaÆZ?îÿÙ V?Œâ»ßŒ?kvîûGî?q1‹~©?œ­&ñÙk?‹–sü$së?ïaYõûÖa?y€Ú¶
{e??eB.Or?6ê
ÿü?"W,;ç§?y"*Žª@qAGN4FGL J2331.5-0258?ëx®+eÎ*ÀM™ìòù‡À;m/®CuÀ<'Ô{ø@ §6…º?ú¹Ð¦v ï?Ó¿²ÝãJ"?Ш $ã1?ü@j‰
Ö@kù«R(Â?ïò6H'iI¿èßvBQ‰5¿Ì/¥ßøù|¿Ù(ë܇ç¿Ðki$Ü®A¿ïÿÿ" 5•AGNbcuGALEXASC J233112.94-030129.9?ïÒڕ¸8–?q ÈIFÑ9??¾÷Y|-F?9ææFxä?t–Å"p¨?pÁBØY»?ïÒÊêø?wKÂµ´?E嫍ԋù?P¤¹!?sÞ='FÁ?tq±2'qˆ?îð
è/?v!˜"˜?iÀãó¢?sWp2¤¹O?žÆ@#ƒ(C?%x¼R¡Ñ?ïu?m½·Xç?=•¹ˆÔ¯Š?(sà˜;g?çX÷åj®?mŒbFïš,?ïm߶"U.?ŽBR ckÃ?VQXúxo¾?Ow´Èv&?Þó¯©j6?"qHª"G?Ðæü"?Šìò²°r?Ruñgšï?`ýl¸Ÿ.?ˆ¤ê?ˆÚBŽ+8?íÎ&®ëei? N³#OÝ°?l1CÊP4è?sË̊6??°­@l6? 7~8Ã?î|¾^
ì?ŠyÜP?JÐr¾JhX?CÈCß·Œ?§ÈØSA/E?Š_0—~`AGN4FGL J2332.1-4118?ÕºîmÜQÀQÎþÖ4UÀ:ÇÑ;ÇVkÀ<{èxú½¡@ûs'
@݇»¢?γ$Z'hÐ?؆~ŸBP@¬}Cø}U@"E¬/ô¿îß´tç?îa{zÊ¡y¿Ú@H%©ˆ¿éeDþ6Ò$¿ïôZ 4"[?ï­¹¬^˜<AGNfsrqPKS 2329-415?î²Å¶ÇÁ?ž÷-?#?oH£ÆºØ7?hFPþÕ?¢ßWD4?ô@`µ?{šç3?¨_õ»±Ü?'b…ðÀ(?Ÿ0è4š,
?™Hj¢Â)‰?˜VÉòD.?ì³·Al©C?¢r_è϶?¢Kƒ[¬?"Ýž¯—­'?±<"EÅ[?›öºý"Š?í¥8¼4#H?'7ÔÀ|«y?—=ÔùÅ?~Zã¼ ?ª
î(‡Ë ?‹½×…p>m?í¥«"Tœ?«˜àE¬ZÝ?|ЗäaÇ?yy
±H‡º?±™ßôù?ªõ¥õL¼ª?ì°{Gkpß?»:;ûƒÄp?¥gº.Ù?¯ïA^ª€?¯'l«MA?°ªpã_8ß?ë
L`<?©Q™4Jޖ?¨‡Ñ¯°hZ?—~¦*?»i´'ÿ\?¥äj"À¾?ê³ï±(W?¤KZ¯>•"?¨†«‡+"±?–M+‡ZN?ÁŸ…_¢z?¢É4^Mà€AGN4FGL J2333.4-0133¿Ïz~á²bÀM)¬îàóËÀ:¨Ó¶ËوÀ<	Äf̽³@¢PE½¤f@[›Äí{?Ð<}>šœ?ÊuqǬ?ú]­	¸æf@dõu|Y¿ïh;ibš?ée·ýä¿åž¸‡›jT¿ëŽäŸQi¿ã=ÓLKˆ¿ïÅ¡—ûAGNfsrqPKS B2330-017?ïÐâVÝîn?{FRÎÇ·Y?J"¼Çy?Bs"Â'|?tJ€ïaÙ?z³¨‡GÛU?ﶼ¾rþ?ƒ.NégÐ?\¦hð[?mÙVèÇÑ?}z7+ÍҞ?|$ëû›×3?î՗ŕ1;?'^$•¹ú³?~Sºs£ ?½fÕQ?¥²]‰Ñ?Œµ‹¼f?îÖߜwd?{ær"·Ò?l¬sCúÖ?RÒhÛr?U? Ç?w?z™ǁ©L?ï"ho€?ƒÖV™UÛ6?`ðÁ{çSJ?Yiö%,?Š©³ÁX½k?'y´/r¸r?ï9ÍÚF'?›Nö³%0ç?n¬SñäR?|!'mû¯?"ðº@AßU?–f·àz«L?í¤—©ÕQ? 	ŸHס?o8Áï?Œûց½?­ÚÅXÆ2?š…™q%"*?ì\D­Å?˜W¿áU:²?'ƒËÁ$ô?sÊñP@?¸Ä¤cþÖU?—þ¦Ø/!AGN4FGL J2334.2+0736¿æÀ!¿S£§ÀIGFýëRÊÀ::DŸlAÀ<3ßTŽÍŽ@}³Ö†´å@ŒÏ¡"c?»ñ~‡ðNÝ?°`u¶uY?í¹Å‰¬Ü@uu‹u•?ïÿyYˆ¿Ùjh~™Ž¿äƒÆÞ÷Ö¿ê${àK.Ò¿å'XýÈ[¿ïÿúŒ"¸'AGNfsrq3FGL J2334.1+0732TXS 2331+073?ï÷ùåù]h?@þO…µX?/u+1Љ?
ËÂê]L°?LÒzSË?@MalgH?ïém̃ž'?jâÚñô>?/	˜œ°r?A9™Ê÷bû?d¡¢o0°f?h9OWAï?ï-lŸ»r?~Y­è?^²ËÒÐi´?Zõ­ ·?ˆKT.k?}?>v‹·)?ïâ•–Þ1?Lӟ<þ?7ç]'&-? ehsýQ?jî~ð@Zf?KϺåæÎ?ïï×HG†?Ut5rìœ?&̧™ˆW?F"F¤q?]wڌ
ùî?T~ŽY¬:!?ïºnód?·¬¥ø$?B"Ÿ¹Va?T(S†à?€Xk8I¨Ú?€ŽÇ•¾Ï?ïGP¿
Aw?‡S˜ç±Ä?j…è?gål‰Ä@?"Å+"*'Ê?…mÐBA%â?者ˆÓΟ?l-{GÐÍX?QÒùÒ¶f?=bãn>?ƒ3kÒ†?jÏC¿ÞTòAGN4FGL J2334.8+1432¿åáاmåÀF1(bõ˜žÀ9|G6v¾À;ïXÒÿìµ@XjGFˆ?þl»o?®Ï†C.0ž?¶'Ëïت@æ¥×Û@;FY€¤Ö¿ÀFdé8¾8¿Äa¦ù~†™¿áéàÙÊQ¿Ü÷jU¥#¿Þ¦YÛéuO¿î$…á*ý°AGNbll3FGL J2334.8+1432NVSS J233453+143214?ïûµ.ºAt?.ËFu¿N§?®®/=t·?
Rö³jgÁ?<êÞÂ?*"²iCú)?ïédÎòÓ?i©6îÊ;?1HŒ!€?Aô!/€½?drzc)?f·ôa‡ø'?ï°¾yLòø?x/DMÜ?`Zò¯Rp?lpZì½?sIò¿?rÜN´"Ñ÷?ïÙ·6ì%?QUäø5…ò?(¾ù³f"i?ðõí°ù?r^†¬*¸Š?Pæ¡Áz™?ïùƒl0ªÃ?:|Ûz›Î™?"v2ÐÃV?J?܇©?ETÁÒÊ+³?8å| ´#?ï»q'?'"+Ú È?ABâ'NÙA?UÑMÏoJ?€#õ"zCU?ºŽ1ŠªQ?ï"Jß!c?{7•'SÍ?c¾JøOž*?j'vmA7]?†Išˆû¯?vt³p,PR?ï¨úE^Œ†?k—V+,ið?;/gÃ?(ÂåÂÔJ9?"é53­™?køMd#AGN4FGL J2334.9-2346¿Ù'j;=ÀRÚøßzNÀ:$Ú¯ä^ºÀ<aJ©q}ò@ÎRв_Ž@ܹ>z?»)9à '›?ŸÐb¿¤Œ?à"´/Gh@®òÇ2Y?ᅴ÷Aë]¿è%5y^¯¿æª>,‹y¿äùw_Ýá¿ìxá=G3¿ÏüƒHÊI:AGNagn3FGL J2335.6-2342PKS 2331-240?ïÐTmYc?iЌÉÌB0?P5•±?AXÇ j÷Æ?sÓȨɌú?g/Јê…?ïÑôÙ)k?u&tiT?G^îQ¶ª?PØÈâ1Õ?tQ/-y?r(ñ÷m?ï²P'µA?pv<ÚhL?ZQşýÐí?\Üîy¹.?€!¢Ð™œß?k\=|
Þ?ïÇQ?Z*e?Vo@}:<¹?TQ_±%l?8™³6zs?wCM4pà?TZ¬Õ#É	?ïuÄSgÂB?")ªmÜ7]?g^%´Ie%?YOaÛWv?Œ·a¨'>?'€õ°´#ò?ï‹kOüŽÿ?Ž-ÂRlÖº?Y)øÌõ?ivVø ò?Š0Í?Š~{òCó®?ïn½ñEZ±?Þ`W2‰?d=PÚÄJ]?dR0	'?A/jé½O?=óÏDÊ(?ï_Ê瀓t?uԖ®Ljý?oCK¤,;f?Z41d×?9žSµ?sZ6Jöc–AGN4FGL J2335.4-0128¿ìÎ셵ó(ÀME>>)0{À:\+ŒuĨÀ;öȋ­@]ú͑ë@	Þu?Ěº@ƒ'è?ÓÖX¼¯ž>@
tBâӟO@´r€s®?âUT€_὿ä‡"Ô@^•¿å°¤xí¿éëâ§)¥¿çç™!#¼¿ïõQ@9AGNfsrq3FGL J2335.1-0133PKS 2332-017?ï¿3žµY¶?ˆŸQ5ôûâ?fðïæßð?m Ṉ̃ä?tí¹a•$?'D:Ä+{t?ïfؔߩ&?"ÙUÅz
B?t¡lÚÈZÇ?€o@©2?‹ù$V'!?›=d¾Ý?íZ?ÎæÇ?¢ ½ÎwßÅ?˜Ð¬¤?èiYŒ˜'?­÷"+ã«?Ÿ.Aн™¿?îF{ÖKaä?…	áçLf?uü©jZ?\'X×®dn?¨ôÃ"Ù²?"g/'ú‰¸?ïyεÛÀ?­úÕh?ù«>?­ó?}Cw¤?€rXÍú†Þ?x€<(ŒÕ~?î‰<‹õR?¬Ν	û&?†!'Ýþòf?"Úr6Z-i?¡ãڌQRE?¥õÑjû¨V?ì»ËƒÝ¬?¨€°†Éqô?¡í¿Øø«?•›ï—ús~?¶A¹'dJ?¤)EÁ\?ééô0ÂY?¥Ê¢6\n§?"Ñq'YO?ƒ{†ÄäÐÁ?žzJì/?¥"l?Þ@AGN4FGL J2336.5-7622?è5jôQRÀCõ¦ZÀ:d"j]kìÀ<‡ó×ӑ@Ä%4ÂÕR@«ÈÛ¦"d?¼¸€uÂ`?"þcGÍõ?Ôà´`Dc\@¥¹z׿è7ŸS—Ø¿Ï"na‡"n¿â2/ýô¿å"~Z#¿ãÞó`4s$¿å"à\÷RAGNbll3FGL J2336.5-7620PMN J2336-7620?ïîB¤xµ?PúÅÁ³C°?5@ëe·?%êá'Á?^+·‡ür?Nõz¨ÞH?ïäùúWt†?k5bsûÂß?2DQ"¥?@y%Ão·Y?hĝº?huJžû~t?ï«·"7?ua5œftö?Y</Çˤ?cO‰>m?ê³'Qc?s(0ég?ïÜÏ,A¢?Nl=@"p?Cá¥=ÅÇÍ?$³HÛba½?n8j¬P"\?M…D×r¡?ïÑ`—?hJöU'Àá?O²YçÙF£?@Ì,\Ñié?sYl\ƒç?eÿ—;yµo?ï¦
*Šî?"àÑ¤?Cë»1ûÔu?RZDà%åX?…=ù«Æ?ƒ'·3ÈV^?ïl"1~/ä?ï̦}î?aԍ1¤)?]7M*Ÿu°?3)¿øñ?€¾BìáV?糧€Ê?l¸ñ·‰Œæ?X<ÔTŽ?Cs™iíÑ?ƒ¶ö"œã?l
À×ÚÊ¢AGN4FGL J2336.6+2356?ÖÑ7{ºÀAê]yЦÀ:'ã8IªÀ<}\ã/å¡@sòvŽ+@‹4*©ø?À¬Ëxº?°Ö‡X¤\?ñ´)¸`.>@'#uP5¿ïø
ñâ?ïÿ*'Š‰[¿å3¢Câ-¿â•"z›¨¿×Ⴜ]hç¿é؃""^ŸAGNbcu3FGL J2336.5+2356B2 2334+23?ïÏ´4òÈV?f`xÅÓ?HyaÑ?=Œµy
?u"ãµì"k?eõ T7?ï¿ÝÛS?{ƒ¹€Ce?M'7hØIÃ?QÞ!a»8%?|lŒ'Í:?xŽþÓâ˜?ïU߉F?tï7TXÞp?a\k´y²?]sÒ£d`?‹Ó"ü¦Î?rÝ|èöÞu?ïkœGb®æ?iM/"7<Ä?n…l œ¦?Tx üå?w"™&?fSM»Ž?ï":˔#Ê?{^ö¶ËØ?aloˆú?YŒ¬®™ºâ?†–Gðþ‡?y%
è¸F?ï0'©úԌ?"*)4ø?`µ·†»X?f¼Õ
,9?—ì4å#"?'ˆÿ°‰Q?ïӧÏ?"ú9ÉM±ý?ll9U¶g?j"᧻øj?™¥]—B?'úP°s2?î¢õ[óW?ƒ¾«Í?ˆ?"y?pY!_›Mþ?¡nš~¦6&?‹©þSõüAGN4FGL J2336.6-4115?ïñRY­àÀQHÙŽuyÀ9—ÇÜ£¦À<$«:«Í@Ã×öv"\@»tÝøn;?±dáVÀ{?½Y(ÿíOh@	Sü¡¦®U@zßøx¢¿µ+Pæ¢`è¿ÝA3¼pQ¿åO°!Etÿ¿æГ€ÐÊÞ¿åWõT«S¿åOß;AGNfsrq3FGL J2336.5-4116PKS 2333-415?ïøM¦üم?@Pí±8A?8&QÿßØ?ŽªƒÏê™?KB^Q.q?>|²˜"Ž?ïðûtn֑?c"ôÌv·×?+¾Lz=V?@$=*ªì?Z¨ŸjÑ?a2ú•"=Ë?ï¨þíÂvï?{…'…ˆÄû?e4VƒºÕ?rú«ÙY?€s.òðñš?s}«øÑîa?ïð±˜`Uø?< ¸Ñ6µ?'¾Š!tA°?9Ó9	©?[¤þÇý?:Y>¯\w´?ïóAùþð?KÍḯ*u?(Ï%Á×b"? ¡3šó?Vb'Gƒ«}?J
²Ѥ´?ïÓMYq'Ç?}3¦\JW?8•b½$× ?LZº›þW?tÏý)ɐ?{Šû«æWø?ïQsö¥kè?ˆ­;Ѭp?tõÂÊÍg?yZÁԝä?Ëƒ´pƒ¢?"z:3¬?ïÛWËT7÷?YkE¹i¸ì?;¾ï]Đ[?*7okÇ?p˜+IH¸?WêÃòzAGN4FGL J2336.9-5859?êÈm(f?iÀKÐ<³åuÀ;VÅÓ´G›À<Á ªšrÝ@/ª›õiy@¸™aeu¦?ÜÚ]-W§?Í·Ÿ©~+?çx˜˜Ú@X…ïBÃt¿ïª'ñ¶'!?îa«IQ¿å¡­>¼ÿ$¿ä¶+ÀÎð¿ïÿìêy…þ?î9æ@;YrAGNbcuPMN J2337-5901?ïÄKÿ‡à?q'ßþ8BÒ?Wûb[œ¸M?O§Ëµ…â?x?\F]û?nÆsºx§?ïӎóÖÚu?tçøbTñb?G^Üi<‰?U.}våC?sLª¦"é5?q~N9Õ?î"-ámK?•‰XIfR$?‡s­¹Æ'ž?"ìér«áH? ña°ãÑæ?'ùŸ
>??ïر¡Å"{?V×νæG?C™¬鍐?2"庠9?q3ù}—ñ?U+Ó¹??ïaW_|+9?°Ïø¬¯?iØâTRx'?l,#ÿ¡|?™÷ÆDß?‹%å¸n*‡?ïv¢óyM¹?'‰OÊm¡ï?a "BnbÕ?y{Ê-ïW?ïE
W9?ŽZȬ‹M?í'0Èäy¬?Ÿ¿©­ö¹S?kq–"â	?‹'–££'H?®§:¢*qJ?›ÅïˆÅ~'?ï«W'õ å?sHݾ³k¿?F\ìk·]?D×öЈˆ?ƒÄZê?rqlO½)AGN4FGL J2338.0-0230¿ë‡öÖ-ÊÀMàÐÜüŹÀ9/{T44»À<
ª}í@tÐ%Ǻ¿@¸t »ÌÊ?¬¾lô-u?«ж'L?üu`4=þ@yFCcA¿×Â;cÙCS¿ã6M½øô¿æTŒê^®¿çç¾Àš¿íäŠÄÀ§?ÆP²ŠMÈAGNfsrq3FGL J2338.1-0229PKS 2335-027?ïò:¦ÞÀY?Q—ñO˜V"?1lP$‡?!«j\—?W/žKU¤?P¢¦k`·€?ïí·üd%?g/X]é-?/¶"/øE?A+`$Í&?`M"Ý02?d3Û?ï¹ÐF\ŽT?s?ãº`ù¿?[düsvv×?]‰™'ù÷"?|>ºZ˜I?q¡qÇqñ?ïñé3à­)?@:lìG%€?1†ò¨?[k­Ü?Wæ§ÎÂn›?=Ób%¯?ïäß
<?_ó3êÄS´??CëQ¼|?1>3™}ƒ5?g8x…åj"?]öãôÒj?ïÌ$Ú¼
?€Îêj^Æô?Bôt·H'É?UÃ*æù=Ø?w"ß	¬!j?~™e›Ä'?ïuŠHm×õ?ƒp`̞?d`Þõh×@?dN×gæç?…68ï?'-#I£Ù?ïׂg›<(?dØyãJ¯?KUËå½Á?@å{ö|Jo?pہ›v¬?aтÑòt©AGN4FGL J2338.1+0325¿Þqn¢u
nÀKX³!ž¶À:ÁêÃê¦À<AF¹!õ@…F/9T@óMAÒ2g?ËmÖݜӶ?Æ	ÃbÀ¿x?ûI·ôÎs–@6+™Þ¿íÀ.ž£ï‰?îjA¢a¿8¿çöLÃ'1¿å{î|Iý¿á©Šrµ)B¿ïÿýç!éAGNagnPKS 2335+03?ï­¡Y½œ¿?tßoãyùÌ?^UH}èy)?U¥\š[?€Í{\a?r"ÇÔ`,?ïŸX."µ?ò°å"G•?akˆ|?cü$3R8?ƒãtYx"?}Ø-GȬ?ï'Ÿ ?ƒÞ*ÌÁ?r$YîUò?l	u6pNü?–"u–™¯Ë?}Íÿ³o%?•'h?{ÎIãÑ/?xsp'y6?`¬ž?¢1& u"c?zNe'Ø^?ïHÁ"™áy?Œ¿ŒuÙEã?sbÏ¡÷Ê?nL­YÌCu?'¬-Û?ˆÍpQDíÐ?îåáÿK?›DŠÐQ\V?vKèÊùP?€LjDÈ?°ÓÓïYS?—ÅZɗf£?î*sÿV6î?•ŒUmZ?…ECÀ™ï?{ùpzٓ?¨ov4?" «—º?ìYÒxw#è?™'ð¯–`?Ž¤ÁèXžœ?{˜
jí€?¹\ÓþÍÙp?˜%ÊËÝèAGN4FGL J2338.9+2124?èÍ5QÀC2¹^Zÿ*À:»ö»³ À<UCh4œÀ@_FrÖ@(è6ú?´r4ûµB—¿‹v±ÚzÉ?Ø&IaÉ@(Çí?)?ïÿ¢âîwA¿à"-F<$¿än$Öyù¿ÞpDAùJ¿ÙK"\Ðg¿Ýô½ÑâAGNbll3FGL J2339.0+2122RX J2338.8+2124?ï"L+/aJ?˜Î§¾+''??8
Q‰B&?648I4È_?Š34Ê\æþ?˜·¼U—r^?ïßøZ"þ?k‰#Œ‡Z?4Ó¶KX$y?@ït-­™ø?mm/qi?hÇ9zù#?ï1ýK£J%?'jÍêrp?U¿-`aá?U¼Î|£2U?˜dc½û´Ó?'J¼"å¬?ï»%hwì(?Z´ÇFtß?Kò?ÐLdõ?.çtÖA€?~ï¯h2 ?YòŒØt?ït{]L?Œ]•aš‡}?OòSÍ&'6?Dž³‹L$Z?q¾Ô¹?‹­l —X¯?=t³9?…βÿ;÷â?E²ÓІ3?T±cþjÉ3?ˆÃƒcQ}?"ç;²	‡P?îŦ·Ü?•Ž|ô·g?`PßÈP[û?\a«SCé?¢ †ƒùZ†?•]Ö %¹?ïC[׎"?u‹ø!1y…?c20£9 ?P-Ù*—7?•)Žpzú8?t¸NùªÖÏAGN4FGL J2339.2-7403¿²¢÷QGÕ³ÀE7~ŽÒÀ:—âà4‰À<yyRژ@X*"~&Ì?þ¤(hÔÕ°?¶äø½–xþ?¦Õç}¨!r?ð˜í×ßO†@o[¸7"l?ïé`ŒÝŸ¿âÕÛN¿àÜ<ÁÒGá¿ÛOBŒf¿ãy«ó8qa¿×À
6Ih)AGNbll3FGL J2338.7-74011RXS J233919.8-740439?ïï%»Œ™½?MßTGœ†?.#6òªf¬?-8_Ÿ?]ð"Q'=?K"íí…Ç?ïÙ¦'O,ì?py/F®ó?9cUø}Z?D€,w|¬?q–¶ß©_?mŠ¶	a\¢?ïµ<ºñX?nCèƒÕÂ?Sb»ÞH^?THßqYÿd?€Dyò¬OÀ?l"́O?ï­¿ ÅP	?ZØë$¹æF?X¼î¾P;Ž?7¥M›D}?x™órZ;?Y{>¹õìÃ?ïݶ¶Ø;7?^¢.›x\?By=xC?4dº0 îl?m«[?Z±ç"æ. ?ï,";>?‡Î•Íý¼h?L‰Ÿ¯30;?VåÁ¸üÿ?ŠpÖVIŸ?†f'9,{Ç?ï‰>þð?vñmq™´•?ZÿgÑåÙ@?Kn•R˜ÄT?ŠPŒ7ð×û?uY3"Ñf¹?ï*
"¢šÛ?x\Ó"ÐÝ?mÑÌ&»ÖÝ?S¼¢"?—©.»?w "ÉmAGN4FGL J2339.3-2656¿ØÞ9õLÑHÀR}|o½'=À;oˆ"xÐÌÀ<Évú2`¥@í°°ŒzL@Wª¹|ð?Ïå5¤Q®s?Œ°'¿7á?¿ø¢~¶_@»©äÀ^?ïª9ú͑¿çôÉ_¿åÕ¾]ž@È¿Õß/»Y‡Ü¿äÉï•N±¿ïéõ!T¹kAGNbcuNVSS J233917-265638?ïñSÝLÌ·?Pl«4ÐX?#ƒ;,&?Í­€Y0ö?ZõDlÃÜ?O}ÁêIù?ïÛÆßî?rvŽzHDä?@U´–Ô=?J\^˜AJè?pEä¦^?p]±äL›é?ï—ëßë@?wŒ¯îË_?Rœ;àõ?DúõÄÝ©
?‡±‡æ­[?vÒ8ß'ò?ïäà¹á4?Jù½Lșþ?'h~053Ø?Õ3L¢Ïk?i¨½ød›?Jl×d8°Œ?ïܝ"âz?c,#Ɨø.?2ԅ‰ç0?&;‹,/?pƒížË%?bŽ›l`.?ï©©^úP?‡lÇo€?KüW[T/g?\Ïÿä?ƒÕó%ãD?…šÐøÁÍ^?ï/"[/â­?‡pÊj_å?[¡(-ïp?W¥¦‰Á[<?˜a¢@[?†Ñ¬LÓ?ï°>¨œæ?jÖ6?C˜?=r äϦ?1'$0Af?ƒÅ]?jW_\6Ú®AGN4FGL J2339.6+0242¿Ü—gÔêAlÀKÀ"`ÑÀ:$رÝ]>À<+ÉMì@¡ÑÖvï¡@GPܑeî?ÃMK7`êQ?É¿?#€c@ù«ó8qa@
£E±,?ïܨAÓ	'¿å~Âþ—Ë
¿ç¡]]SBG¿èÉv7]d¿ïø[#*¿ïü'«@‹AGNbcu3FGL J2338.7+0251CRATES J233930+024420?ïÍTj*L?¬Š˜È(ò>?pü'{¯Ü!?¬–ôØv
?`²pè6ëé?S©†C'?ïu¦ÅÒÈ?'‡ÓûF0?q«ÃÔî_?'ë¨ñUŒ1?‰Àl˜äÐÀ?†þØ0ÚÈ¡?$gq?€N5°'Z?q¯«îu?s"K¶?"'·âÈ?wë³îµ¤ð?îñƒò#¯™?uï"2'?ä…"È~ð?bŊv+¤u?˜Ý>òʆx?s1†é?ïdž}÷Á\?"Q‡-Ǔœ?igX³b?".›n¼éX?o_ÇËhñ?cCSŽài?î¡ì\g½‡?¢IÓW²AÒ?'<Q,'J?¯@—AG?¡R%ð25:?›¿"ÁLíÃ?ï)T³Ç©^?ŽT­$'Ï?€mΆ«–I?€M×Q±Õ?'ž'Gԑ#?†d|ÖFG?ìÔÓ«aÿ?"¶¥¾Ì÷?›§¯™Ñ›ë?'¦Å/Ù9R?²o|
zcŠ?'ªÌ©MAGN4FGL J2340.5+3854?Ы²d°sÀ5ëVûW÷À:á½ñg·À<…üÉêš=@ Ih«»M?þó•:a%?Èîºu\N?©PÃß4к?äfg=%û<@1" k³?êÚÛé*Ñ¿ÇÀ[zO&"¿é´ò?øé`¿Ô°– ÀÕH¿Ï^c¸Œ¿êg%©ôçAGNbcu3FGL J2340.7+3847GALEXASC J234042.83+385510.7?ï–*2r\Ù?tƒ/™?C~(¥N^é?59ÌÑpz?‰=æ3ÿv?€¸ŠÅ'%?ï¿<Þؒÿ?x9q*w?LaÄ=e	?UÌ藫È8?|Ýätж¸?ve[ú?ïNí«ê?'ÁŽ&ˆ"Î?_¨dÉglh?Os×cP6/?"'Ä?4žB?'mËÏ:ª?ïTOOs†?ol֋ö?\µ+V¬a?Bž¾R¨ÇÉ?"³ãYǕ­?nÑ³oy?ï4-Ãv{¡?'2¯ºG´?Sö`ƒo?Gà üññ(?˜:å°Ó¯Û?ÓãJ^?ïV4c<Ó?ŽH\‡ŒÉ?]­?m?j•rýÕVª?"hÊK_œ?ÎAýÜ?î¢NÑkº[?•™ôL1u³?gcꞹzö?b97IwS?¤dÔ?,Ǧ?"ñ2)?`à?îãÀjz?‹~åúup?r+¶ìéà?b¾!×tÕB?­\M("Ù?Šñ7²–71AGN4FGL J2340.8+8015?좂^>¤«@1Ðx·¡Â]À8»ZôB\œÀ;œ—ü
§ú@ Øf3Í?ýmlš]
ø?¦/ºîí‰?·ø«wènê@Qš&‡S@uþÕ®Ë?ï¿t¿Å}M¿â¯LåÄ¿ÜÂ~_o׿ԈB#þÀ¿â\ʵ›X¿ÞR+[xv´AGNbll3FGL J2340.7+80161RXS J234051.4+801513?îTPåv?®S:0Þò?'JW~wm_?¬+<sí›K?«(ü¹K?›ÃG(b¾Ÿ?ì,Q+¹
Ë?¹›æûÍr?®PIŸcm?°"»žÕ)?®ê£¤ï¿ê?«ÎOaoº+?í#2ø®Z¤?£ÉFT'?é´ƒ¶Þ?‹Êö{o­?²é1«un?¢,«fHg?èÏÔº4¢R?—Üðc?±µå_jÉ¢?ˆ…ËՂ³?ÃåºhŠò§?"*ªY¢Œ?ëåù2u6þ?±
x¢H×Å?'Mˆ§Œ?›CÈ®diÒ?¼|Ô@MfÕ?®4?iû°á?ç_Æ<v?ÇõAS:\?ÂÿÇ9Ô¦Ð?Ãòü#	£?ÀÞ¼{gX?¶ÙТd?ê¡ï1.T?±¹(à[æ?—Bt^,Î?'é3P]'?ÄÙ7v0UU?°5^ä­bP?á÷ g ðr?§MÑV4Å#?Á¸
7¡? Iï‡=ʲ?Ó5¸"힐?¤À½Õ8+AGN4FGL J2341.8-2917¿ØžeáØ£ÀR¡quŽ!–À:öä/À<±páêkC@~¯—ݬÄ@ۀ©Þ‹;?Ìs‹èÖî?Àx)Çόñ?ñàV·œ¹à?ü¢òÙPé§?î³àֆ¿Ó¬p¡RË¿ágž	jâÍ¿âBl¡"ãø¿ïÿF!!Ä?ïù‹a~ÖAGNrdgPKS 2338-295?˶;*?tåiüõÊ?fÖù°ŠhÑ?akyä[('?aŽ•Ð{t?pz–Ûù?ï"$d¹=#?‡–7á¯?hLnÐ8®E?mAåmw§?"ãË:ѵ?'ÆOv]þ?ïÆž›G?Š'g_Ûhä?7ç×!ú?º«qq«?"kK#™?ƒ Ið8µ?ïϖø÷Å?z+º¢4"#?vŸ€¥8?`.?¦Ü"À?™E¥?ƒèF?vðØvJsd?ïXȄ¤Ñ?…² ù ?{ü—ØÑ?u@#Ÿ­?Œ@`÷^x?µ"Ä—"?îÝl÷=þW?¡ÁÅBýO?|`x«Š?…û ©5?:C!ŝ?™öËHÊ;?îŸãÌ(ô&?'K\ÇA¢¬?"¿"GRÌl?ƒ+‹´R§H? ÑÞlwñ€?@ñí?í4‡zÌé—?—ïùaP3?‰Âúý;ô[?z6¤×âi?³#dË©»?–¿EËrKûAGN4FGL J2343.6+3438?ê/'¼³O"À:.o`àëhÀ:+'›O|À<>9E›ëƒ@ á{´×7µ?û=uâlv?º…™\‡ëF?°ZKÐãݵ?ö T3]û^@Lï‹h©b¿ïԍöÎ(?ê`=X¿ÂÝÚ%ÐÊ¿Öe
{"Ý¿ÞÝh»Ö/w¿ÅWÙc¯AGNbll3FGL J2343.7+34371RXS J234332.5+343957?ïòQvnq?L2+wž©´?)Ǒn³ý??÷q]™T‰?X$ÜȶDM?J#ル ?ïè#¯ ƒG?iççÄåð?4>;à?B¬ÑV·®@?eT‰`»¨t?fBé;ZP?ï±*?ĝ?l'݃m!/?Su©ÒPM?T=Ìk·^Ö?Fºô8Ç?iªï)‰–?ï÷G'd|?bF9Ò?S/ÀêÅËò?6ž6{Ù(?‰œ6•¹š?a_eĔ"Ù?ïå•9¹?ZòLM2{9??OÏ7â?1€¾|?güˆ'?Xn¡ß"lè?ï¬Õgc?ƒØ–ñ$ñ(?G[ѰȂ?Víª/ña»?ƒTééçœ?'\!ÄùY?ïyvªðó·?|í›ymª(?[â¦ÔnÅn?Y²©çþÉ?Ž&hÝCz?zlh²;¿?ï
É?µ³½?yς˜Ðã´?bWsÕ?P'k\_F?›ûäbKÁÎ?xÉ<œUóAGN4FGL J2343.7-5624?î'ÜqÀM(6CˆëÌÀ:Íã˜Á,†À< †TBw@Â>%Õ|Ÿ@ç<º›qá?ÀÊ¶Ú ¿–rŸj`h?Ôì¾Ü-"@Uf¤S1?¼æ+ÿžlx¿ç¶Â3얗¿éÌVè'¿Ô¼Ì¤ˆàå¿í=Û,áàZ¿ãYyMÉ·oAGNbcuPKS 2340-567?ï÷-Žâ0?CH¾ßFš?4rAµ²Ìí?*¸óO†?I¤,÷Ó?>êZ*QÞ?ïïX-ú V?fØè'
?)¤Nê¶?8¶UpÀ.+?^/£Štê¹?c¦†üÛ˪?ï¾é1(äG?r×c©µ?T"ö¼žM?TµÏjÃæ?{"'Eëø±?r )Áõw?ïó ø¢Wr?8-ÿ *¼?-,\ †?ÀpwŠ@B?Uƒ"R'‰?6»ôòcE?ïð¹±<"›?RÐÖssýï?C5Í\z%?:,IXo%?U	†bÈ1?M<œQd"?ïɾˆørÔ?€S1Ü|³?8d~ªÒUÙ?Lð¨õ$x‰?yšs‹¡_?~êi|½¦?yáԂ?}sn—üK?]>7H˜¬~?dq*ñ5?‡tÚ¤Oæ?yÌÁj:›?ïÜwN.ûÛ?Wx«»ˍ?Git¬¤?7y>²+ŒW?m®T)'Î?UÞµ³5AGN4FGL J2343.9+0546?ïzéîEÃYÀJ¢pCßÀ:ª¶P‰…OÀ<iDo›™N@…Ã÷¼º@%`â˜ç?ē['÷
é?Ò­Ûzº†N@	»ž ç×@J¨;rò¼¿ëoyȸ?ѼB¦m½s¿ã
,kü¿Øò.Ü"¿éΕßе¿ïÿëÞ
òAGNbcu3FGL J2344.4+05491RXS J234354.4+054713?îô´`¨?•'ÖïŸç?nŒ‹Ð>ƒ?ˆ»Ðiÿ?úá†bó$?…ŨTî$þ?îí‡jB ?©—Ù.'·?"ÀaPõ2i?#Æõ—÷?—îâCÎ?¦÷KVŽ®¹?íxWŸÏÍ? Ãi©j[¹?¤€ªà=íÌ?™"S;!¥?£ùÛaIe?"[Y#$Ú?í³{ Bü»?†ŒJ¾¤œÖ?"ŠU*•/?uŽ'žZ:Š?ªƒ#cñçÅ?'‹Ø²|s'?íZûFŽ?§~'hÈÃ?¨1®? ‰i1=?¡Ëû?"Ç?ÕÚ\?íuÅöKï?²«ó5Ě?˜²KâĕM?£Çà='¾¦?¬J‰àÝp?¨I®ò1»X?ëä.§™e?¦½"ù
‡1?¯ƒ×Ykø? •èZØú¿?±ZD¤]?›`Ÿ²J[?êx¦V¸ÀÉ? ìß%½•?¨¢;Lù4?'yC…2PØ?¿é¯¤¦p ?›ž÷ Œ²=AGN4FGL J2345.2-1555¿î˜æ
¶g[ÀQ¿j@»À7!–5dfÀ:þO'åJr@Þ_ùÎj@E}àÖo
?'àQ—ì}?ºW±þÑgø@&§lH'¶þ@ª#
¡S¿Ç¼€xá¿Ùòì;}·¿â_Ï=ÀTï¿â?êÁf½¿çø@îݘͿ糝쏋AGNFSRQ3FGL J2345.2-1554PMN J2345-1555?ïÓ78a¬?jèY†â?Gv×?D$Ãr÷¿x?su£˜e"ò?h	œß
ßï?ï¥~~	×?"@/¦þàZ?YzƒiÚw?rÂQ®ÔUa?ƒîÐNÜ?'󮧷ƒS?î"Ì/b?Ã½þ¨?Œ{ž"ñß?'\à—	:t?ŸHùÐdÉ?˜OÚƦL?ï­s.¤?tg¹¿?Kþ÷Œ˜]€?F°¬èLKZ?'ûóÁÜ@w?r]gÙù?ï(Ú69D?|gjIÚõ?V»üÕ^?PÞ
ƅE‡?…ÞIäßïè?zööÄV?ï<"ræ8?¥wQÆ÷>É?xߜ)a8W?Ÿ4Y0Å[?'5·p9ææ?œtÚ¤v?î‡Xv0*b?Ÿ¨Š0´}?ŠsËZ°}?Œ2æÝK+? í…ÉÀïB?œjÈÿ@p?ï&ÔNf.?L.ÄÈù,?^†Æš7?WÃp]…?™=ЯQß?Žã*‹1AGN4FGL J2346.7+0705¿ÇÍ´Ô2œµÀJ.XOLnnÀ9,¨hiuåÀ;Ð֟´eÎ@ 51¯=?ýŽ Ç‹Dl?­-=¿—ôÃ?–oBᄝg?ìHÆxõ@íÈs÷žˆ¿ïÿíUÙPi?ïþÝöÀ¼¿âðûµîcö¿Ñ	ç_u0"¿ã£—I]A$¿¾_ðÀòÎêAGNbll3FGL J2346.7+0705TXS 2344+068?ïÉñ3Ő?t¼è¥Ä?EÛIĒ·?=ßäŸrT'?xdŠ­^Ç?rîc!™Í?ïÕ*è­º?z( ¦ä?FÁoåÇ-4?Sßæ*O?r']ì>Š?vëaÆF³?îÇú¯ÖiP?•RÕ
XÆ$?t¶Sµ?yÞn¡"˜ê? þ>3íBc?"zºéòã½?ï®™RnY?z3Ô{<k?pM5Ùåg?TŸ6mЕ?šVäÿxºŠ?wÜË£§‰?ïœý¯Ì>?"r"@Ž™?^žÚYä?a­ùvCÁ/?"ìÓ­…—?oþ@oN?ïŠ!wQ£¿?Ìµ·½?Xž]U 
l?r¸ëçÌø?ŠcÖ}Ëhç?‹ßPäÈ6Ó?íÈ;]Ne?ÉÄöãÈ?~lÔ.âáÍ?}Ѻ"#X?¯®³Ñ?œˆ!ãZ?î",û‹§?'X2Pr#Ø?0gN2Zù?m"‡	]ǒ?©ñÃZÀèS?|. "AGN4FGL J2346.7+8008?èØÀ®[r—@1 -à
À9º¶åÚºÌÀ;ÍÂ5fê@¦7Õ.p+@…³ƒO«9?»(
æª?ÂK²›s8‡@iS×@úȗ^¿ïÿÀ_V&Ó?ïÿHkÇÏ¿äçøé
¿å÷BÂo¢¿èy‹!0Ò0¿ïþõÎÇúAGNbllWN B2344.2+7951?€œŒW?"Ûž
'a3?'¢óX©o?"Ý2SAùþ?y:yÖ·-"?tò2D[]?ï)î?›&àÕÈgñ?…ƒŽ"¡Êû?!´Fd£?Õ÷äj³?‹I®'îŒ?î4pÎÞ?˜Í\4vc»?‹ôiÔï?†¤^Æ>P8?¥»ý¦ò8:?"ůHÃÃX?ì×HÞ‡?‹Ñ±SF9?¦6ø)eâ¯?"2¬?+–‰?¬Tyô –Ý?Ê,"šÄ?î'n.R?¢§•8Hâ?Ÿã€¹Õ¢? ÖRmÇ??‹ó3v¡ˆV?†û´@ä̞?íXÉX+ñ?µK/æ8ø?¢…|:¿î?¬©Vg9?§ååÀÓ?¤;gÄÆ9?ëÀtÉDpâ?©(ïÀö2?¤>ÇHÐê™?˜êàîs¹×?·Üö™Å ?£I('ñ4?è|\ò@Ç?£Õ]ñÌ?¼Fù ž? Ç"TBì?¿×_&Ó?˜S{ AGN4FGL J2347.0+5141?ïJñ=D"À#Ԕ-IgÀ8* Á@§À;h$Ÿòy@EY,ìó?ûñ«#.Ù1?lÊ{QE?¢µê!
Uˆ@TÀ%@hbå}rÇ?ïÿ5À+SÁ¿ºcCÇ* ¿×j[h†|¿Úï ^Å2O¿à
͞ƒä&¿×*kÄR{AGNbll3FGL J2347.0+51421ES 2344+514?ïOøªû?…|C«X?2'›´ƒM?/¿‹
C]?‹›F¿@Ã?…(ã›gÇ\?ï\¤Ì†3"?š÷+}<{?G7VÜL;?Tá쥢iá?"±«»•Ÿ?šªöÒôró?ïÃI|†õ?'/ÞËðw?pIïvŽ?xË.eÔ?›%ã̲?'Ž/º#›?ï`ùýtW?sù`nŶ?aµNüFrå?EŠE©Ø±?'ª2þ`ìË?sB¼ž?îã"¹W³?šŸêƒ¦o?Dñõ
H1ô?@°…?PW?¡z›Ðȳ?šXfOh"ª?î|oý
y£?®t ‰úu?W´75™e?eùÆ\E¨7?§{_°Šd?­â—Ôõ?îÖèi,á­?•ÁQ½Ž ª?p×4¤^Y?yäž(ã6»? þ"ûˆê?"§î¡&äm?îæXhe³Ó?‡õJé_	
?mQË¿#žm?WäfiSÉ?ŸŠ¹yUMÝ?‡4³$ªæ:AGN4FGL J2347.9+5436?é'ÂŽõ®Àƒ#5.À::sí7¦_À<4¨ÒÁ'@!†Š!×k?ù?yB=K?¾%ŸÌ¹–?È'?Š¤z@ÁvÂÔüF@RbŸ\|-¿ïÿéÅ+Ü?ï÷‰8ùEÒ?ꝡ»üñ¿ÔŸ4£ ®Œ¿×ՙd•€Û¿×n:%âeAGNbcu3FGL J2347.9+5436NVSS J234753+543627?í@G0ž¶í?¨¥A@Ý­Õ?'–ø'år?ŒÍ!±U¢õ?±˜oY6ú?¥¨XM«?ìœ7•?¾"Þ0?g®­5ƒs«?yKŽ¸õ?»JŠcë¹?½|f üm?í±Ê*¹šŸ?›ž¢wK¬u?'XïJ'"?~>Ù3'iº?°&ÂÃO?šaí'eO¯?í¿tÒiô?Œº3Æj­Õ?ŠÏMAé?o˜Ñ'Ûª?¯¥ÿ
Ô¹\?ŠWäºÌ'‹?è¸*tÛÓ?¿´¼"LV"?¦ÔôD¨)? <ð†œY?Çj¿¸«ò?¼n:Êp?èÙq‡?Ç«"$xÑ?€ç1²•?'0^Ä:êÓ?ÎêcœÃ«Í?Ç6	ý.ê?ê,lü=äÎ?¬![eô?—úƒu]'¸?'¢üS­?ÄNûŸ·Ú'?©Í'Ô¸?뇯çT ?¤­sa¡†?Œ'g30}"?…™\Úaåí?ÀðI².?£{@ËÙòAGN4FGL J2348.0-1630¿íBg‡è[
ÀQù2‹m†ìÀ82Îí8}À;]«›úœê@ݾ•Q‹c@QþÍ?¹? ãò¿`ä­?­H­Bî½
@T¿Z'È@Ïîq¸)'¿ÊÊ«õ¼°¿à.‡'?àÁ¿å&ŸÔœ$¿äì~ÃÕW¿è%Ë5ó×Ô¿é™ÝŒ7±AGNfsrq3FGL J2348.0-1630PKS 2345-16?ïí'²e\??Qk±DØ?#Åó;Ê?XE¶gd	?a›î&D}?P榙-¢H?ïïáÁ?i¼?e`ÎxPÐ#?,icnLŸ?Cb=Rjä?\¯QdÀ)Á?bRäsp‡?ïœøF?€ö>1%SW?]Kœæ!?ctmƒoÅ?…"ÅÃcÚ?€Ñ4'è%?ïï¿Ø"ùn?E™Ýøsb±?;:¼>.¯?hÇÇ?_š¢Ó‰?Eêýˆ+?ïÏK E
?nRc'ˆ«?1*+רK?'8¦Ý iÍ?wBGí·?má¢k?ïÎ ìrÒ?'Ÿ{þw˜?>=ßÂ!DÊ?_®ùûH©?wJ%¢?€¦JÒîn?ïl‰ÌO¬ï?ŠAªÐé?eA¼¸^×?pʙc5Q?J%¼z?‰
ϲrh?ïÛŒÞÔ?`gG«±?,‹•fC?#?
è?q™
RÜðS?_Ŕ{ÏèŒAGN4FGL J2348.1-4934?í
*¦OhÀPlvJßøÀ;,ägô À<¨¦¹<Í@‹>âéÅ?ý‡RÀ—4?ÞKþzÄÂ?åՏHÝ¿c@úÆ[¯S@	M/ê©V¦¿éf™£U¿äÀóEšN¿ånç´¯ ¿íc¯!–'Ê¿ïý³¿µ?ïûžaTƒ»AGNbcuPKS 2346-498?ƒ8Y8?µc"Û g?†´M›²'?µn›î!?hF«¤uÎ?këyÛð?ïªç·ÏB?†ð`QtH?b¶ýào†Á?o}Ú7Ò/?€˜yYðM¼?€¢#ÞXô¹?íê›íåSà?žX­lêvò?'&]üyQ"?
æ?œ?¨C#n8?šNŤ©1?ï¤<,Mˆ@?oï¨tsß?Jl®…ÑŒ{?;Mó†HÊ?…J*[:?mÍë›8Ò?ïžAî{·ö?šôP;?pC—¿ÜÇ¿?–­£Çø!?€M¸ŠÂ†Ž?…òQ?CÕ?ï(Oz½=?¡Ý&«L-?x¶‹K/?Žû/n$þ?"ôIN¹²¥?™µýqh¹?íG«²Ê7?¡kýgûó?ŽHûtꈁ?IÔñ¡}?±ùƒv9?Ÿíþ˜\?î÷ôd°­?ŽŸe…‡?RÁ@\¨€Ê?Q"îJ4à?ŸÕ_dáÎ^?Ži®îóòAGN4FGL J2348.3-6049¿Û"P{\[ÀKT¼M"ÉÀ;¼ZÔ–À=»µMTG@lR
¾Ú?ùžõ#-+²?ÞTñÿŒ<º?ÜÊ¡yaë­?ùã÷aËÍ@氛"Äÿã\ܯ˜ß_¿íQ±k뿸4Àüßå¿áõN€ìy¿àÓnÝ-m!¿ïÿ:=°AGNbcuPKS 2345-611?ï'ú4¨Âñ?¦8m(Ô2è?`"ĎFù?z¢\£$uì?‹®|f?¢ùaÎx´Í?ï­Ñ;"ÌH?€µ&2±½"?W¡>=MI|?^½Cç'AW?—‰Vzêé?{úŤ~•Ø?d\˜T?–2Y‹ºóV?yés´Ë)?yô™†*§K?¢R¬‡Hce?"Šz§A÷?ïŠAaÁˆ?g°Oä§Þy?@¥DoB­?,m©$d°?ŒpõFÏ®e?g%²–?î¾ØL ®»?£þ¹Ø&Á?tk¦X¥ Ì?pæ;V?ï.?¡…v¨1?¢÷dg=
î?ï±µˆý.?œ¿¼üœ´†?f¯
ëӏ•?«Û 9V?™3çêÞ¦V?˜ÞµA:¾à?í"E‡†¿?¥†
íöµ?ƒÂßiV¸£?…'3ã–Å?±e|q½2?£öåm??îÔ¡Qѹ?…Ò¦a›Sî?B'¬µ©Á?>9¹Îaæñ?¢k¤=âc¸?…¦ÆpϖAGN4FGL J2349.2+4535?ÿ1
"FÀ/ÒmÚÎîÀ:¥ub'¬À<
È°ÞZ@—"Òã]@"Âqÿø?°yÅhÕW?²öwÁ½o?ñ/N6ĸ+@
ªúý·¦J¿Ðõ"¡•'w¿áþ˜h¿äÊæ¾:Å¿âz?+Žú¿Õ£'{šÖ¿ïÿX¥³ƒPAGNbcuTXS 2346+453?ïíÉmX]?sˆiiÿ¹»?,‰‰-–á?8®ƒ	?`múŽ¹Ý*?r¬'¹™?ïì
mtÖ?ià
'Ð
}?'>â•auç?8ΤIj?b¤&-ÅÅ?hbï~ôl?ï²6¾­û%?u¯Ó´öÖÜ?OÏÞA??X00Á?.'¬pý?u¢!?MB]?ïáý<[?J‡4fÑ??/"Ý-´R?ß¼œl{‰?l–6Ëá›?I¦:T?ïߗ!;±S?d¶žWÜo^?;ÞmN¬Y?3©o3Ib?líôÍÒp?bøiã§?ïÀ)ˆ1Ù?"[-~Ó?Bt´~ƒùA?TK‰ç?}œ¥i
ç?ƒQ|‹*_?ï}\-
»f?»J@XqD?V?ÑDù?LĀfO´þ?á{ŽËó?~Ò×Êu
?郎WaeÌ?jzXRP֙?Eƒ™ 9ª?6ïÀ¯÷H?…|º&16?j,«´$AGN4FGL J2349.4+0534¿ÈN(yhCÀKo?Rü&À:`%t-ÏFÀ<KÏå†6@¡-g—>@ÕÓ;{×?¼ÿØè¹èD¿"©*±.‹¯?Ö%Â1hWØ@	â²r®?ïV%;"뽿éàp]‹ …¿ãßvó|d¿æwÿëÞ
¿ç…æ>7ô
¿ïÿÓ?,» AGNfsrqTXS 2346+052?ïóAØ´ÙÞ?HÎNòÝæ^?0"X»þß$?ðÍÂۋÙ?Us¸·Ö–[?GBo7Oؕ?ïÜÚù'¯À?l¬i©\E?:¬¹á/[?B1Cþ ·?oÏoXñ:m?isoGTM?ap÷ÿ?uYž§†?TXÒ܈ºû?TI÷Üw: ?"ÑM?Aí?t•M\¼²æ?ïÄ]çւ?WWžX5m@?I'òÁ_w?,˜Vã¬?zÎòé¯m)?VPOŸä°?ïԉ|•ý®?lñɐÀ´?H×¼v¬¡?;Ðh?r Júo?jÇ·Í«ÖÈ?ï›ò>ÌC?"ÎύDÂ??LGѪGâ?W-,»wHb?‡>ó1š¿¥?ƒLa£?ï9Í¿ö?ŠK'L8ÕÄ?`^Š>"˕?YìñÀ''Á?–ºåCV»?‰ëÿºWK¹?ïTCm¤"?uWŽ^¶ol?bIkÈQ'?Nª3Pmþ¿?".rqF??t`.°óñAGN4FGL J2350.6-3005¿Û¶(pŒ…ÀSA5Tu£À:#5'Ì÷À<k‰öŽg6@ÙZÂC[õ?ÿÅ%Ù®\Ÿ?¹U%¡OE? ¯&ɘdæ?ç?–¹‰$@\ü؃9[¿éµ³áC|W¿ßè|U»ô7¿ã×jµ€€¿Ù½Ü¡u0¿âf˱CÚJ¿Û²Ø
€ÇAGNbll3FGL J2350.4-3004LEDA 3231681?ïø»Vònâ?7çºVþ4¶?/Q-šo?ïlåìgÁ?I,º§3=ñ?5v|,¥L?ïí&B<þ?f[Q å@ø?*Ò«£À©?;OÒÆòš?a,"`9°?d=;ž•?ïÉð÷ös?hO9»míÚ?KxWō"æ?1¤{!UB?w˜yh^©¨?géqGö?ïÝÄréµ?Ori]k«?0LÅ|a³?j	C•.?pwх\¸u?NU€•kó?ïóz}–ûý?Gè­Dx]?,ë¹Ø«T?ð˜äÄp?Umž¤öc?F9(-a
?ïÅ©)Pþ˜?€&¹…x̄?;¢Öք?I~T!ÿ±¿?{q=ñ"g…?~Ó20¸?ï¬*Øh-Þ?o—ôå›?T&ymŽ?U"Y#YaË?'så	l€Ö?lÊG߂$?尿©™A?kŐ¸]uÅ?Dƺ̚3—?5ªŸÊPV*?…)é&Z?ka¡š>çAGN4FGL J2350.9-1416¿ïý²àJÀQ»y(àÉÚÀ;lmî$nÀ<ÉÎ	îü@]šÖZ•"?û6*^x[[?἖S"ûË?ÜH$".q?ù/H!×Á@~DÖHÌ¿ïÏBÈÒlI?ïòX!ªÍ¿ÛïY—Œ¿á\à
—2·¿â ¾z#³¿ïÿ>9 ²þAGNbcuNVSS J235111-141557?ëÍۅwM¿?Òdq8|s?'Ì¥SGH?ŸødS‡S«?¿7"ó?ѦKøÖ?ï­éȹ S?"1åý¶©¿?\r©ßš¬U?f=Sež?€÷8"D½Ä?€›÷TüÚ?íYv+³ëˆ?£xõŠ'?—ª kߐä?"D½åy"?®"M­f
? mà_$"?îÊò»…
?€Tö&åS?h£ÁÚæ?Z)•ƒ•
f?¡Æ˜+4«?~K8C?íÒïÅ0‡n?Âáæüñ$<?ˆ3Ð~Žú?"`ˆj˜?¬ÄB¸×åi?ÁÁ"ü7.Ò?ï5‰>—7?\¢Üþ$?rO^ÓÆ\?‡#fÊTñv?"»á+͐?—BAlQ¥?í*÷;›"?£cXhAŸí?–Ó&Äjµ?"¹ü'?°ó|tPÒ? Žr›"JÄ?íyÝFöG?™%µäVjì?gÔ÷½ãA?eýÚWð?³rn¾Œå?˜õ…¹ÎÿhAGN4FGL J2351.3-7559?ïYŽß¯ÀDJ­ÕÀ­À:G,å;YÀ<d»±òUó@ iÐ~25?üµY~ —O?¸É­6Ú]?» ç¬!0§@HIёX@ØÔ2Ü?îöúÓpTý¿â¸§z¡‡¿ÑQÐb©~¿Þџše¿áú@¨f¼¿áz螺jÊAGNbll3FGL J2351.9-7601SUMSS J235115-760012?ïôV͆?EðÏ4ÆH¤?%ÿʳ¿uü?¦âM!?UØŠ­<?Cº%eR˜?ïȹÔïÓY?u"[¦?Hr,Ãÿ«?P€:à/F?x¡§9Õ5¿?r˜7"òë	?ï·Þ³Õ)?hZö/û`?R$݈pwB?<Žó±Ë?‡n½µµ?fÿÜ_åt?ï\UÌ÷P?kÏIF+œ?i°œÑì?G©\"e?'Hß7 ´?jK˜8™?ïégÝðó?UIï%|è9?;‰ºÂ£ô?,˜¼çf³?c€fVñ?SFÁNw-õ?ïII¼{_·?/Õº©?]ø,MÆp?dM@ø³"‰?"÷E°ß?Ô®ø¹UE?ï€z¬Íµ?zﻞ·˜?[ß"Ø_?Q_©}!F×?Œet:Ô?xÝ®Ô	É*?îqÔpQ™?"×ÿ*ÎýØ?{'Ÿžx?b«'$1c?¥reдÍ?ƒñÊRâ	§AGN4FGL J2352.0+1750¿ï¢ò'røŠÀEd9¼º0À:¤Ó‰pÀ<\Ti
à"@T6üÁ\+?ÿ:F"bH?¼'uÆ«¡?ÀÚ™Z"†@gMú^ÖO@DVä"=	¿æK¿[o'¿áK+­,ôU¿à'ÉEnŸ¿ÚwPCKã¿éø@îݙ¿è,ì\µ½AGNbll3FGL J2352.0+1752CLASS J2352+1749?ïò"¶~?H¬šÌ("Ã??
Ç}7?6dÛh‰3?S:Ÿb?B7ëú¼ê?ïÐÍÝîÞ?tYMýxŒ?C¦ß³Ò-P?PJvÍ¡£ƒ?u$51l¶ñ?qÂkhù?ïº>–™?t…Fi†'l?XJº²o³ª?dZÔÉXÁ"?|ÎAþ
rÀ?qS'Ýþ/?ï™çÔ~á¡?bKõƒó'¦?Y8I3VïÓ?:äÃýQ7k?†_ºŒ¥¸?a—"Ããb?ïâWAʤ?^øþ÷ç?Y@
M^3?S$(—"p?a¹Þ¶=?P¶z¼'»?ïwÌAv?H?-cø?Sc
wô?a6ì[¡|? ~t«÷¶?‡t՟A?ï†ñ€rÆ?'קÑ%±?hºV¼pýM?r«¸Ýªá?ˆåpYE?~;taô`?îüVhJæ?'¡¤R¡·Ç?nÀ=ŐÉ?[%½'ÄK?œ+U‹{2?34çéŠÕAGN4FGL J2352.9+3031?¼Ÿº@¿IÀ>®˜¹ZÀ;RƒZ'ôÀ<‡˜(€QÊ@¿§·¿tu@íx:¤?·Êóìn~¿¾\€^Š$@…ƒb°@È>¸w€??ïPz¼¿çwåê«%¿ä´þ¤á ¿ä0]ºpT¿è{~@w¿T¿ðAGNbcuMG3 J235254+3030?ïÔX²Ò-g?|Æ靍Ñ?Kܟ˜µðy?H1iÏwº?rXšE=Ý?{­.…£–?ïuíb¦¥?÷Pkî´«?j6ђu3A?w:1|rŠ?‹÷
I@L?‹åÿVjxw?ï	f2[iU?"KåÉ­d{?dѲó±_Ø?lۄO—O?œ9N5{?")ÛÁh\ä?¦1úÆ?‰Âo4ú–?u³à%ãH?_®id9'Ï?¢`eCÇB.?‰OŒÊIœ?ïv#?Ë?'í™Z‹e?püÃH ?qI¾)ŽÌ9?‰øΈc¼=?Ž›~Þó¹ø?îz2zóށ?¦£i3ò·?¦Ð=†?g('¢,Ü?¤ycz@{?¡XI#¶A?î6¨ª¼?›âìÚ.@?}^	Ú Û?€ÑG +?¨é½®­Å#?™ÿú¥ão?ëMœ
šÐÚ?ªw+´Ì–?"…¢o?ή?ˆJ‰£ó³Ã?À8ÛyôôÅ?ªº²™MwAGN4FGL J2353.1-4806?çxꔀLŽÀP‰VC´À:ÉÝÑôÀ<Å
?#@L£Ór¦@$É Èb?ô2â€hE?Á>Áh¼,?ü\e¬,CU@Oš"Ñ
Ÿ?ìÕ©ë të?·˜Jd°¿âzé«)äÖ¿Ü|Tú®1¿å`ºŠªéM¿âB¨@ÑVtAGNbcu3FGL J2353.3-48052MASS J23531112-4806045?ïâHû؏4?V§Ào?H2=F?@i¾å8ÛÚ?gªt¯À§™?T
¼ÙO-?ïР4=?tmÏøÃ?KEŸ9>z?QU|oÐe?tM+•H<?q˜€íã·7?ï"ÅÅÁ?r·>ƒã?\ËUU~V?\³qºâÿf?‡uOA
<?pŽÝž™B8?ï—ÒbÊ
â?cºGûögÇ?jo˞0?KÀ'EÇ?ƒƒ£ø»ð?ašu†ÈP?ïÁù'Úˤ?hEBxÏ?bú)ù¹ïï?Xþ OSkâ?u†W
ç?b!Þ£Ä'Ó?ïuWWL9Œ?xgHMF'?^'÷ TX¦?fß;ÇJ(?Ž×ËCåÑä?¸‰Úðã?ïI5sT`?}Z+?'ï?eøZQ	Þ?`rIû¡ùq?"FU¹jÑ?|zùɾv?îô¸v?}ðíõ¿Ž?h©_¨è²?h¶`Ë,?™•ž­íž?z–ò)cŠÄAGN4FGL J2353.5+6646¿à½",Asà@&QßƤ•À9ëîÑÀ;'F1<¸î@½¡†øØ@õçB™Ø"?ÇéÀãàd¯?§ðd+´Ë?ã—cßM'ë@Áûa4Î>?ïþùÛ"Ðå¿Ùÿ€>Sοí5{!‰g¿ã^«‡ça¿é ÝZ¹‰ú¿Ô6ŽûçAGNbcu3FGL J2353.3+6639NVSS J235301+664243?áWª>‹»?Ì»gÐ?|•/r£|m?R²|Vú ?ÜÞVÄÕ)	?Ëûsjþ?ç7šlc'±?ÁL}呝?–áBS ^P?˜Ûð}ÂR¿?Ð"·=Ðy?¾þœ±.¿9?äB·kwÙg?±F¼eÂÆ?§©²Mgo?—³;ØÓ~2?ԅZÞÙûÆ?°|͓U¹™?ébíå:È?¡:fµ!?'¦Á[°£?käçCC=A?È?p>'ž? ®Ïš^Dí?ÏIª‡ÂE?ÄkÄ»v?Œ>§Z¢bì?‹ž
 Q?çÍò÷®Í³?Äg¨
ƒSæ?Ýr4Iw‡?ȱ,âzø³?¤.Ëæ
?ªæeçDÛ?àùÈø?Ǎ±y4I^?Ø30³ž?²º]§ƒš²?³ûÚ@¯^?Ÿ?gGW›?átk6QB4?³ŽÙF3¿@?àá±^9ú«?¯çÀ"ÁSÙ?¦hu³?‡˜"Sł‰?Û{5('?°%ÔxXOyMIXED4FGL J2353.5-1457¿ïÉœ×¢ÐÀQö¨~8ëÀ;DâΖÑhÀ<Ÿþ­©@ (&VÉ@íÅjؼ?ŧRiÚ9G¿­eyxù?çþ)f*×D@÷»õ9'"?ïîX¾7,¿áËހ("Y¿êà*b)?ê¿Þ"aùð†¿¹ n†,¿ïÿÀéz-AGNbll1REX J235320-1458.9?îðÈýO:?š%Î×ÐI?a¼<ïa?bJ
ûZ£•?Ÿ¯xä$?™"Êb`ޗ?ïµbW/‰'?"q£ £?[Ã^%ž?fÃp°QÎø?~^|­ç6?~؅å+?¾Ù]ï?"åFn¸ë%?l`ÇSÇÑ?oü~!Ìä?¤?žÖe?"wyÕ²c?ïK;÷–¾¸?z'sê]Ù[?H:@*Ñ&Ô?9AýĬ ?•Ö¯Òv?zQv䑦7?í÷™HTÇF?§õ•,Mö?w…t¡M$C?w&¿Iôƒ?­•¼å*?¦ÒyßÝ#?ïo±.>_j?"³Ó!–!?`º×Ò¦?qRÀû3@?å†"'ú?''M·þ:?퇨äÌY? 2

½?³?sƒ6'ÕQ;?udì‰Å¬î?²Š…p}ý˜?Ÿæu^Jü?í^ŸÉ4?›_~œ'f\?er–Å.ÀÙ?]æs'¢ó?´_lÿH$P?›b9úÛOˆAGN4FGL J2353.7-3037?µ‰^ÀS9Ϫ͞"À:7\óöÝBÀ<}:Y˜!Ê@ÇO"L«T@©3]$žE?¿¬Ð6f?¶a·U\ä?ö,û
͹\@¤Žèe¯‡?ï¦Á4éÙ¿ä?£ƒþ'¿Þx¹d»•¿à¡åÎ%'a¿êºM8—÷¿á4ÂkñAGNbll3FGL J2353.6-3037PKS 2351-309?ï™rJ}Û+?€ôþ£?e6?EOìX?aˆdòÀ?"U݋Ş@?xàc?ï©Û‰å,Ñ?ƒf$)0z?a´¼,Î(?g@–÷"ð?îb9¬,?~
2‹¨ø*?ïA:ÝÌy?X
±d(®?ü,›¾\?"9í-ÄÕ?"™Ê…¹°?‡h²m'X!?ïË&É1Q?sçíÈñz?z-cïHb?\ªäêUÂ?–BƦÕÞ?qˆ´Ï=?ï0
Ü.?£e3N?……¿Epd¦?£6|ª$Ë?•7¨¡D??"ˆ±Tþ?ïFª0?™¡êGs?uVŸð?dÅt¬?—á¸ÑŸÓ?•d†É-?î…‡c¿¡?–9É¿?‹¤½;p€?Š.:&Ì°c? Å€ÞÓ?Âõåvœ?íË7,?ÇÚaÅHÈ?»"â
·à?u!f_pÙ?«ßûKçêG?‹d‹ŽÌ³ŽAGN4FGL J2353.8-3911?¼#0‹¬'ÀR?Až0PÀ;	æ~OÀ<Á|Ôfõ@ …±…@ïó»NH?ÑbäRzv?ÅVV"÷Q?óœ}YÇò@Æí­B?íü݀ú}¿é$â7˜¿ä=а‡é¿å^à
AL¿è5é
†¦¿ïÿþBe«+AGNbcu3FGL J2353.7-3911NVSS J235342-391442?ïÝõtO¢?\¦'
~ϱ?K^ª¦]?BP±!Ô·#?l'rÒ.ÝJ?XDÁêmÙ?ï¹RvfÛú?}ɗ3pïN?VlØï8"5?ZÿÛ]'hÛ?}»Ž|Ö"‹?xù#Òø÷×?ïY£êwÏè?€}åt?nödÀZãÐ?u;Ó&Ãb:?ì¶3–?y7ú+£qˆ?ïX9®ç"}?pð\–P[Z?fGp¤¡?IJOAˆÔi?'/çóE'Â?p`ç·¹ß?óqYè?|¦0/?cÈ ÀÆÙ?^{)aL?…5'Pª@?x'$÷Hô?ïHyšÔ5?•ÓºÐì"?h»gíI?s)26‡ž>?"ïnÀýÃ?'©dùåðÆ?îۄˆei¼?‰ª‹»QӜ?z™°˜]?{֝‹ç?é膟h?…'ñæÓ?î1-u•>§?Ž‡çÂ%ç·?uõJâÑ?e€{râ¢?ª.J\i?Ž²ì0RHÆAGN4FGL J2354.1+2720?æèé#ÎÀ@çu¸eÀ:ÖƞµbMÀ<›
ü³Df@x>He"@Òµþ,Á?ːßò?À)á¹mõ?ô}_Üßiˆ?ù§õ
j¿Ü°h}—ÛS¿á»'Á^Á¿æÒ<çè¿Æ6`y½[@¿îƒÏBrì1¿ïÿî' ÇAGNbll3FGL J2354.0+2722NVSS J235402+272328?戾?€"jÌúÅ?`"äq¾?eaŒ]Ùˆ?ˆÞµ<Tç?|±¯ø3¼?ï`0ÒZÖ:?Ž\€C
D,?pŠ•*®.?v@֎\nª?èîÈf?†½ZWÔ1?ï4ÚZT	m?Š£<ÁO·?uŸçÌe?xi@O—?"Œïqz\?…'ï¾QOw?îÅ㏏ˆ&?}~QÓÖ?†%¹·—œ?m)·SÔÁu?œ0±7jÜ_?w¾%œ¥?ïÆ•¸?'¦ I©?p¯•+Ã?kqXÎFv;?˜óáîÚÚ%?ŒÂm˜÷¡?îÂkõÇm?ª7 ÛEJ2?'vùá¢?Eç¶u,?©îQ¥æ¹E?¦)/.ƒÛs?îÕH»ýéó?8É0qH(?z%nax0?|ûBTY
Ã?žÍŒæ,ð#?Œ	D'Z"?íÐ_Jà›?—KqÛti?˜
Áü™?…èµVP©?±̅¦³ä?"b¢U¢¬AGN4FGL J2354.1-0958?sÊyÀQ
Ÿ¸fäÀ; ïܸÓÀ<|ùûA@ŸXŽâ[@²c"úÎ?Ða؂b›V?¼_õÞéÛ?íï8œÿ¨@Ý›ëÙW?î®X£/D'¿èÍ_ߎ›d¿æÆuÐfµA¿ØxÕÔ³K¿ë{¢´¿ïþaå£2AGNfsrqPMN J2354-0957?ï¢+pߢ?­ð4‹ð?JÖ½ÖKß?B"`T4Ý?…Ç´5ÜmÅ?­ó-·\?ïҁ:ð?y}˜Ë€)?R]֐Á?_N»¯ÛÒ?x¤ÉäÀ'†?t–-FfÄ?ïZH9Ä`±?"VÄ1C¬?cEKóKL?`³ªZ'¸Ì?'U$PÇb?ƒ«Í)í£?ï‹îš@Í>?hÿ³Fl¿?YpUR—Òo??p‰>¹ÿõ?‰ÖNÃÁè?gúQús?ï,¡Çf?™œ¿í*
L?Z®›½—ñë?MòU¹Q;?š¯'­ä?™bu³8æ¡?ïns—²§?'¨‡K¢æ€?aA¯p›˜?o£Þ‡Ûd>?	W3ñÞ¥?øÌ©<Ö?îÙô@¦†?
ôׁ&s?jë1.äØ?fõ‹k±9€? À/¬&JS?gˆâ?J¨ßw?†n·cq#
?pÝö@:º?]{ƨ!?¢ê¼®RR?…ýõ¾ÒpøAGN4FGL J2354.6+4554?í¬l52gÀ/¬ÚQÎÀ:¤l™†NcÀ<pÈÜ}Cø@2êm·A@=Û?VW?È)Eßaô?Òð ÿê[@1o† ˜'?îo\k«¿íh­aÍz?ïÔÊ\°?¿åã$\֚¬¿çèŸ8iÿ¿àoUB§šc¿ïþÍ?äF'AGNfsrq3FGL J2354.1+46054C +45.51?ïT«#Àà—?u:ôÛz3?pLZ6fÞ?qÄÿU?'W"üGœs?‹g߆6?ì•æ'Þx?¹>?îNôý?­¿Ø5 E¼?²gö}؁?¨á¾¢AÒÁ?¦x¤·œôI?ìàÃM¶Ûä?¢	ˆ¾Íà? Úðæå·?•°jÛ.ÿ?°ŒmŠgº‰?›ºâêpv¶?éL˜Y?¡*''h"T?º«ÜDíxr?ž/$Š¡¡?ºóVú7¿	?"bü˜z1`?CÀ°E? %ø¦BÀ?… {ªÙ"•?"~ƒE®Ü?¡nÜÚö?š¸Á¦HÁŸ?篥Ö5?ÉßõLâuš?ÅfqƒÐÚy?Æ;'[Â&3?¼¥¤C/™e?¶÷D«¼Âû?ëÏfÑV…"?¦kYøiÒ?¥vësìÕ?˜´Ùá¿?t?¶ÉSºx?¡½®þƒô¯?ã
ù€¼?¯"M""?ó?Çã!¶;ÄZ?°qŠÁ®nd?ËðøI·?©c4t$4ÖAGN4FGL J2354.9+8151?½0‹k·@39¸ºÇËÀ:*Ô2ò›"À<B€'،@D5݇…@ÝÊeê?¤?À.I¼ât?¶y<×Ì°?òF>¢‹±@®õt‹Ã¿Ð-lŸ»q±¿æHdˆ?Õ¿æ=ò^¬³¨¿è–6—k¿ëpù'7}E¿¸—ß/OúAGNfsrq3FGL J2355.5+8154S5 2353+81?ïxÊ«4w?ˆ€‰Tí?m²›	ÇÜ?dŽ¹Ðì?Š"%ó?äX?"´Åv ?ï‹í:šI‡?ƒ˜£µ/Vð?ijàWpå¨?k÷ý¥¤>?†©ù=bö?~Q:3¾°?ï'ÀÙW'?‡ä";QQç?u T'¯B?rxô'˜q?•ÖÒp_??"|V&ÈÚ?ïR"x¹éà?l]9ûÿ\?y²~™@^ç?Wãs"†Á6?Ž…¢v¥?fPA]û?îW=+ãd?žqtžN?†—ø—œbx?zY¨i jŠ?¤æ/xE,?š¸H³‡…?î¿ä]¦èü?œ—[¶É/?}£RïâB?ƒ[Se;CÒ? MOÎ{Kñ?—";ßé¯é?íð½§bQ{?š4^$¥09?Ší"Å·5µ?ƒ÷þÀ•?ª8Üב3à?•s{ñ¿ª¸?íâ§mÓÔ9?Œÿü'?"jNÃօ¾?y/y«?ÆÙ?§ aÄG‰?‡–©žK9wAGN4FGL J2355.7-3351?ï3¤Ý
ÀSzž+ϒÀ:,ÊëK=À<™QþÐU@wnåhz@€öÍ0 ?µŸÍ»4I?Ÿ¼*¤T™Æ?ãa¬ÃB	@õÕt'!{¿Åì]÷,è¿æ*—MŽÿ¿æq?2oê¿çäû¨'k¿å#'@ßÄ ¿ïéþ¡[.ûAGNbcuNVSS J235538-335225?ïúhò¡Œ?C'/IÐՌ?!>ƒè( ‡?ØTø'‰?Cnºéo?@S ¿ô.?ïç¿E¿kª?kôþùQ†?6*ëK?Ft
Pٜ†?ep™û©+?gÆ1_˜öÂ?ﵦÉ
©?s¼ó¿‰$?V¥i;ñÞU?`î!hRø<?ƒA¾ƒ?qg~E«‡å?ïïñn[—?A‰Àó¬e¦??;³BxW?(º?a²†?XN64ž?='+šµB?ïîéU!M5?`:0/Ï!Ð?3^Î7^m?0șòñµ¨?]U¢2zã?]yp'bæN?ï­à'¶Ý]?†O"àì¸?M1V0j*?`Ã;m°-?'´Æ>'à¶?"äà¢ö?ïe­éÝ©¿?†"=STç?b÷æÍõ+ê?eêvHä!á?ëEìoë¥?"ÍÙ^¢ïü?ïÕ߶g
^?`Nƒèú¢??VQŒ³V×ò?GT7<Ê?n÷ƒ#ÊVC?[=À*TÙAGN4FGL J2356.2+4036?Ìd]f|PÀ52¹¯æÀ:"ØÛÎÈPÀ<Z¾ÎÝHE@ =û¹tUg?þْx=(?·0t¼ëXS?ª\Šo…?ՆŸ Âg@ͅþ‡/	¿ï¡ºÃ.¾?ÿ (¿ã'! 
ҿٛÈ]|\ó¿â"c'0qb¿×ïHÂçp½AGNbll3FGL J2356.0+4037NVSS J235612+403648?ï؛#Ô½Ô?_ÄÁ.–½Ý?EeÝÉÀ«£?4¹ÿí'?q²tA}q?\ã12Fð?ïÑËøož?w÷Nú´¬?FŽž[8p?P&YH?tH/çŸÇ?u4<ô?ïv²—uÂ?vL ¤ž-?d¬t$œ?YßÉ8I›Ë?S/üÁ3?sµð…7G?ï=)LH&?pÅN†šì?v±ô
ÁK?VUÙFqð.?'®YƒÏ¹Ù?lª`0Ô?ï´ÿ7ûf`?p}~Ì.?W¼ñ³òs?EÞO'´:?''®½f¬?nû·TÃ6?ïuíôao?3ÜI™0{?W!Ϝž°?g¼¢RR? €Ç`}?3¡"Žª?ï
§¿2kž?"oª8Ìoó?o€ô›k«s?eµ¿Â³¦Y?šZ酕*Ê?'•M#©?îB+Ì6¤Ø?ˆ¾ùÆ5ƒ?‰f¹#êÄ?q
E†D™·?¥ƒÂŠ4Ù?…¨šú}ñ.AGN4FGL J2357.0-4840?Ìó©)ttÀP:ÎÄÀ:ꋨ?OÀ<È«Yµ}ü@—Ì±Éç?ÿ¸j1Í?ÅÑH#w)?ÁèN2'úC?ûq¹_ã•?úý¿é+ÿbKO¿ÝŸæ+]Ò¿ãµ…Q8¿ã"ñ10#´¿ÚNÖ½;ŠE¿ïÿÚ
¢ñ1AGNbcuPKS 2354-489?ï»
Œ9Îr?pê2MW@?Q£ÍûM7?H́'ë?~ÆYö«j?n‰N<2ê?ﲈ{¡®?ŠB÷w‰?Xnåꖾs?[ýM½\ö0?€PIŬ¬?~'Î'·`?ïl\˖³?|ý'ÁÙÅ?j·æͳ3j?o¸‰3Cóü?Ž:ÕcÖ0|?w"/s6ãª?ï{(,?x³†Yõ?pSH®šß¡?W«'¸^â?™͵݈?wD
Ù¾Eø?ï^†ÕéùP?ƒ÷b=ˆï?j­söYԁ?bg€íÈ?ÙvÁaæx?VÐýÏO?ï*σش"?™?ýK8ÆB?p‹¸®Pk˜?z&_÷H?–ƒ!Wõ|?–1g$ö[?ïúk»\?…Gªí±©?p˜M!xs?l‰Á²î ?šZ«/3ÃS?'¿­Ôõ'?ímªjÄê?–†ƒíSã©?ƒ}Ãg¯ÏÙ?uU"Q?²"ôAàéó?•çã(ƒØAGN4FGL J2357.4-0152?è|p+¿ªÀNÏÝ~Ë·úÀ:z–ê'°qÀ<zô/è%@LN†öª@ñ*_Oð?ʪ¾ZO?´‹õÈ|Ü?ñ"4 ½@;ª%-?½¤Òݲù¿å_×5ÜZß¿àHBY@ãö¿è6±•+v¿è‹D× ef¿ïî¤"‰—ÄAGNbll3FGL J2357.3-0150PKS 2354-021?ïÜVå?
?f#•Hã†ë?Fé0ªÿ%?`?‰šØdÚ?n5]YHWõ?\Ò¸?ý?ïß;o T|?m¼'acŠM?:uÞËÿ?C—Cð¦?muÔC<Ùc?jˆŒQ?·H?﫧NÊ#¶?qrÚÁÊ?]=+H?d•WÉHn?n‰Jîó?kœíÝ Ö‡?ï¹Vá
K˜?[T~Š‡?S6£&íÏ?6)4â~¥U?~†æË
øl?Yžyÿ%´¢?ï¡Ýí¨ÜÐ?xô9Ò¤r$?Xb̳•£?Rًòq
?"|CBL?vöג¼ó?ï•íxí?ŠžpH0~?R«À``?a`>šÌŸØ?ˆdŠM6Å?‡³z¤?ï\DbkÁ*?ƒ^>©{?k÷üY
?oÇlùÝ?øt(B²?€ þÐǂ‡?ïMòÕã?x?*Ew{?d•¾ç¡J?QïÆáÎ)*?"¯k¹tq?w&ª9¡ëAGN4FGL J2357.4-1718?ç—%屎óÀRˆÂß
A1À:;<ó¦UÀ<C³aÁ»ø@ ãÍJ 4©?úü´=Š?¿ÜhKBôq?©÷#́?îmÓ­'ž#?ù ¤äüD?ïÝÍ:°Õö¿ë>³>±@ª¿Ø}[À›<¿Åó.ö¸ƒ•¿Ýþ‰Þ:³Z¿Ö›V½ÑÝ-AGNbll3FGL J2357.4-1716RBS 2066?ï°²9ùuø?wOáŠa&è?A‡¤AŸ?2Œ«ÄU÷Á?'º÷/x"?vâßü?ï³³Ä>?ƒVÁxñÛ?YbgœI?bh(,¡Î?̈́3ª6?µýáÃX?ïT`ÕWá?Š¬£'=ÁÞ?gÀy½f>'?b‹`ˆæIõ?šÝd¨(Ü ?‰_㎆ö<?í'¢1KZ?ŠÆêÙ©ßJ?uAf¹ßÀ‰?[…öäuM?²#<ƒ¤&?Šf….‡æ?ï9M-ZV?ŒÿÉ8¢?X³
>pä?J|Åñ‰L?—A%~©?Œ|_‹¦Ö?ïE—­ƒ?š5[òé?kTiiT?x,B²»×B?"í±p_j?–ýFcÒè?î¦eô•X?›'ú´²?q–вy«8?kwŒ»ŒI?¬"¿‹…TŸ?šxïy ݃?êCãIí¤?£xXË+®?†zM‡Ì?urb2"?ňѵ¿¿ô?£q	Û¤ÔAGN4FGL J2357.8-5311?îþ8
á¨ÀO
LÂPrÀ9³v/1EóÀ<B­Vœ@œÂ†!í'@…	¿œ?°1¶±W{g?"°Y_ÓáO?ߨ8ã÷5×@¨(#µ'È¿ÔDx $ο槹ž¿çK|€.8£¿æšD¿ë^œ£9UŒ¿ïÿëJwAGNfsrq3FGL J2357.8-5310PKS 2355-534?ïôÕë·?…7ПWX?5ÄÑ_ÚD?eÌ|Ȏà?PäÆHM	?‰Œgù)Ê?ïóWH™Õ\?bÁˆÒË43? ÜD¥¨›í?4WáßV?W5戶û†?`ÜáþÊÄ?ïžg§:?'`Ÿ¸!±?Z¦ó'3"?b Ù\Ý»"?…'G­î¯-?,ŽÊ¤Ñ¡?ïý‹T)q?0¬ßvç?yX¢Ú8>ñ¶Ÿ?13•öCƒ?Æm³ü?ïô'Zƒž?PTqêqÒ9?3‡$¯Åæ?'üŸÝ_Ž?QülDèŽ?Mwä¸?uh?ïÕúÈހ©?|öõáq?6w…é;?K¢°;ŽC?s›#-hÛA?{-³a×¹w?ïdîW>³Î?†À«ÃÛW?a‡5¹Ã?cRp¨ó€?'1R±ž`7?…Щ×þyÛ?ïù°èÃù?;¥
fd±j?uÑ'½´?7—×3?EÒq%f?90KõffïAGN4FGL J2358.0-4601¿×f%õn<ÛÀQÇ%ÃßÀ:UŽ7£À<›£í°r#@üaŽQ@Õ8ü Ïï?¶Ml€—ü¿ !`!þ­p?ä)šÞh*·@f÷1OXX¿Ý§dŽu¿ä³[wN¿êeøí½]¿â¨¯à-¿áîKØE¦Ó¿ïÿ¢­>'AGNbcu3FGL J2358.0-4552PKS 2355-461?ïù>Ú4'?b³ð˜fJ?&s©}sw?­ÐxK…?Eg¬ï
ì?b˜Ð«ZŠ†?ïîÇÅJL?e¥¼¶«Øs?'7AòQ?9ʶ襇?_‰"ÁÖ3?c¤Õ+Oíß?ï¸6ÿ+ÕØ?rÈ "$n?Vž7£YZÀ?]žÎä^vÉ?~<òvïéd?pTI~‡C#?ïöþodÅZ?3s0½u?#²¿Ìïýþ?
¾q¸'?O"YnÀz?1á.óµäÎ?ïñ82\¯À?Vg{Qi…ÿ?8N"²Eÿ?0#@jå?W|x'2Ô?T"ýº5M?ïÅþ©°H?€ØȒXB?="~Y+…?P.'Åù?{'c¯otM?~O3döj¦?ïŒ[TÜȐ?|'ý[m'?^è'Ø.w?dŒ~fTù"?‰mº*¤=?yüdˆ¡iê?ïå¥MyQó?Uý¯{¿?@µ©Ä+âá?1«±âKH?f-GÕºXÂ?Rø³É†G^AGN4FGL J2358.1-2853¿èpš}!òLÀS‡óõ"À:dü'¶vIÀ<œBÇû¬´@ŸpÕ*>m@ žÛøº?Àv†š
‡Ó?Âø » ýÑ@}¡›Æš"?þYÖ)ÂÇ?؉хCKY?ꫦ!r™¿ç49ÀGƒ¿ÛÎó£PQ§¿ïÿ½_œr½?è[¨«AGNbcu3FGL J2358.3-2853PMN J2358-2853?ï4 cÖFÒ?­Ž2†…­¹?sśãÈR?tŸ_I›8?"»'ɽ?­"
‹ñʺ?ZˆÈÍ?§\'sù|!?ìQ«?˜¡©Ëzn.?š2œƒ…?›¦${ç*g?îqAŽH`?˜•YH9¸Z?‹'©"ÌJþ?‰-Fd\XÃ?¢
'(g<?"—y€_æä?îǐ°?T
,¨ñ?'®äLJ?x¯@÷`?•o	ìöŠw?vUXÔ,ê?î3÷*TL?¨"L<9?"Àĕk™?"Àäèöš?£4-¯¡p?¤íƒœDSH?í²Ž?¹ZŠq'ÒF? k+$Ïv?­ö£ë—?®kîšåº?°Þf[Iiæ?í†FJO? ^ZK›?"¯,È2á?ŽBÌÍ0qx?­ÇåP_›?›
³.|P?ìÕGöõÑd? =,K³?§œ7mOp?—ÿG`v>I?«•äUÅþS?" bØ»
AGN4FGL J2358.3-1021¿Úƒd'`±ÀQE/Ÿ¾wÀ9Q}˜²
À<,ÄFŽ@jÉۀĶ@å:Ü?¯ÁðOÞº‹?µ\â?`ú'?þž"_¦XÅ@­Ô3É[(¿×Ų'¸#È¿ãðÝî]@M¿éR0^—ÿ¿ç2çHy–¿ìd¾ÆyÌ¿ÚäVÁ­´ÚAGNfsrq3FGL J2358.2-1022PKS 2355-106?ï÷)¥÷ß?A²´çÝp?+lÀ×·x@?EÄýïÞ6?L~<(ÞUÓ??.Ä4UEó?ïí`!—™(?h™+é'Î?-¦ôšö??¡Mq:¾?`Å|y2Óà?eÐûuv¸?ïÄ
5µ?f¨&Nš)#?U¤AaÍç?C{3OÞýh?x‡ê­Ðã©?däq «'Œ?ïödÕ[€s?5ÈmÀ =?,Š"Ç*@?A\›l´û?OJ"{CaÃ?3lÓLòÌ?ïðæ+1uÞ?PƒGEUs÷?5m‡9x¸Ý?'¬¾€w5™?XØGEŒÀ?Nt@¾ó¸T?ïLj»áÿ?8'fmæl?D4üÚ±9è?Y?@k?yµ'æØù?~ô›Z}fÀ?ïšÂ&籑?x3ö2"?_
Ðií‹?UϕrL1Š?…n,\€?vªUÀx?ïå-fj˜$?XyS¨D"q?F2ÊuÀçe?8žK–þ,§?eEæÕ¾¹;?Tã|ûþ(AGN4FGL J2358.3+3830?ÁH>)¨½EÀ72"áÉ´À: ôX,À<HÜ}Cø}@®Ö€Õ¨i@R:¸b²?»hŠØáƒ?'-c÷‡qµ?ÅŒ:
'Ö@
™dôÌE=?ïd' ÷¿ÙLo"È&J¿æ#׶ÿ†¿á'‡N={¿ÛMh=¬¿ê#¹B¬LûAGNbll3FGL J2358.5+3827B3 2355+382?ïôpÌ1?C¹ýŒ™Ñ?':[ò†ä«?Î3‹`¼º?T7n'ê?B›{‡U"?ïéãb•»?f1ºÊX3·?.´mS
yY?>ÍÿùåÞ?d1Á}"z?c¢ÿªá¾?ï·]JšM?q0ýYû?Q›G"5p?<hm{?êˆ÷[ó?qË
S?ïÇ:±×¨ô?U¢V±Y€,?G ×Á‰?(Wž_Ö(Ï?ynŒ
©3?Tál'2›«?ïëXá÷	?QVvŸe«Á?6£•˜'ª°?#øvÌdm?aÒ«l؀í?P!%ž~œ?ﶶ7´ø?¢ÝW¹ñB?AQ'´&ÿ?M›+S"Q?=YÆû?èè¤S8?ï‹ý¥Ãڜ?x?'†ÁÍÛ?ZÈ>½"ëx?]­nãåy‹?‰§Ž°Ï™š?vÑ
'Í?ï_‰ì)é?u:c'¡$'?`œ
eFDJ?IÀî
c7w?'ûA:™J?t‡½WȖ˜AGN4FGL J2358.5-1808¿ê¿ï]ŠÀR·D»ó¡À9Ø<Ç0«™À<<4ÿ¼
b@mS[?ýЋö–Ë?¸Š×´ÝAå?«à©^Ä£?õy²X­@@@tÁï•?ïä‹?Ž¶<?ÁK°B'—Ê¿àÞ¬É!F¢¿ÕçÓäC6¿ßMJ 4¨Ô¿åÎAvÂÔüAGNbll3FGL J2358.6-18091RXS J235836.3-180701?ïØߥËÛ?gV'6²Ù?<¡ÕîJ"?0Ál2¢y?qƵ|é~?eÐ::o"Ì?ïà~ÚóÎ?oC±.X|?<á>K'xµ?FÈÀ×µ‹«?kÔY"Lm?kxáì+PS?îΪH?|;
Š"r?`³$¶+"?eÃËÙÌ&l?‡d»B@)V?x±HÆ¢L?ïZ e=?o¸`"B"`?a)—®<?GlL Bm?'–Ì#žYŒ?m÷'ñH‰?ï¸pËUd?y±wí.ˆ?QŽrt̼?H†®C6¼?cö[#Ú«?wG´¤«Ô+?ï£ý5Jd¨?‰o†ý^Û?R¸Y`?ró™Ù9Õ?"©ŸTÂ9?…}­Ä§ã?ï9"^Ó©?Š‹Ÿðp¡ñ?j"=F¬ì˜?k¡ú%?•{³7P?ˆE"¥<N¶?µÀ??‡"Ú‰'ª?rœè²Ÿ7³?`c¡äô?¥7™v"?†KOÌ«p°AGN4FGL J2359.0+3922?ÝeôC¼ËÖÀ6cÓ^·E|À:bylÓgòÀ<7g0Â@Â	O_@é~¿\¢?¿y$?`¤A¿'Å˞?ÑB>éÊ´@
M|'¹Ø¿âïãÂwß¿çѓÛêw¿âÄ´š¦ßÓ¿æ*Ac¿Þï2²¾.¿ðAGNfsrq3FGL J2358.9+3926B2 2356+39?ïö>åæE¼?E9^ùú¯Ô?*½VKóyi?.?çZ²?P*‰nü?C?Ttu&;?ïìS=ܬ?doK½BÁ?)üR埛2?=f;=c­?bý'«+š?bu´gD??ï¨èþíÂ?w\…Ö²în?X¬'vø–?\\î­o&æ?'é€À7p¸?t܊´Á>¬?ïÝKþh?P9J—Ä
 ?,œ ͳ–È?
ÓӀî3?pu—ƒ­/·?Oõ½EaQ€?ïërÌ.û?X^®d|?@q)kKs?5žUÂײ#?`péZú²ñ?U86…Ö¡À?ï¼Ã"·)?'BúÌõqž?;CÖôQ½?J«›¨¡oU?éü­˜°?møÉ-o ?ïS3<S©‡?…'g,`»?gði?mè]À†2¬?'¸ºcl´?ƒ	Ø.÷W™?¶ÚG4?ozFÂXû?E${ÁMd?5îø"Ñ?ˆ¾J†"ŒÈ?nýü2~¢AGN4FGL J2359.0-3038?ïÖ¨©éÀSŒSâÖÀ9ô·ˆ—é–À<;'&¶M/@ o"üT?üÈÄ3¡?´ ëóX§·?'«¥''"v?ßµ<ã5D@œåT-)?ïþé+0/¿ã'[ßú¦û¿Üôú¸îI¿Ô="_ÑKã¿ßQÞú¡Ç;¿Ó·'¸¬"XAGNbll3FGL J2359.3-3038H 2356-309?ïªê5#´v?˜<'jpî?Adž>\ŝ?RåeÛ¶#…?"/(ØØq
?—/S*þi?ïØ)ž?s{®<ù?AÛÎUWÕ]?OÈÊæ²YN?q»q¦ý''?qï£üEú?ï5¹bŒ½?†&-ùV{?d	y秸y?UøVuzþë?–Ǥp—©?…¯í‡Ç#?ïOAµh=g?q5•Ô6ÿ?Zj=€}	´?@§åÎÒáß?"q%yd¯}?pɾC'ã?w:Ái?"y–V߃à?M—~›6?H>"hW ?‰ªKÞôÄ?ƒ³¹ï
3+?ï£Îr$›Ò?†Î@ozÄê?N°æÁžÁs?Z©Éº	+?…!UÀœÊ?…P¯" qƒ?î<þ•"Ñ?—u{ÉO5?qjJ¶Â=?iR]K.Ú?ªÍf…#?–­É'µÃª?îU杺?Š"rhFH?nÞÆÅ?Yí²ðŠ›•?¨·Ìâ%·e?‰tהè4%AGN4FGL J2359.1+1719?ÑR#¬`#_ÀEâà"&þÀ;5áAÎ×iÀ<µÿÚ$@À€ŠÔÚ¸?þfv÷®!ç?Ë©…ïm·?ÅGФÕN?úÀâ³¾ß@¾ivf9¿ë‰¤>8Ió?ïìl5ç¿Ë7dpB¿å^"ñ¿×h@zi¿åƝ]É^ÙAGNbcuNVSS J235901+171926?ïÂ;ßAÖ?''<Yønç?Kì• Ú\U?eqëšå>t?{d¥‡h³€?s-ŠÌ?ï½ÔL{ŒF?w0¿³-BD?MDŠóÆí¿?RDxèb—1?}mH{A†\?t1Ê;¾H?ïnw®|™?{›_h?e µoG'd?héì#qw¦?ç¸Y&?xˆxHó?ïa±+·±?j":e$]?a.?6G˜?H«dqÛß?'¤¨Õõá?iB]¶ª!­?ï Ï`zê?|À™F8L»?ZÎ@´Šë?NƒEdü'?"znp~r?zå1¼s_ß?ïA" 4?'JÖIŸ^?a˜ np²?r'V©2?•›
…Ql?^Žx÷?ïíãÑSÎ?†]"~ÔP¸?l%…}‡Z?hizvúlr?›Ý'ÓèÜ?…BsOÕk²?î~.LïÐ?ˆi}+«¨°?mùÄ:£³-?`¡ÖgGèB?¦={ÊFwÃ?‡­ÿƒãŒÈAGN4FGL J2359.2-3134¿àîė°F•ÀSsC¬ÄðÀ:Ê§XžþÀ<Œ5¶›2 @üЁ¸&x@¯¿%D]'?¾šòŠ ªÅ?£ÿk@Ñè|?â%Ûüëx‰@ÌÆ+$q¿±=´€û"	¿ãB©D1ˆ¿ê-b
ç¿æAµaÌ"Ù¿éKŸÀûs¿ïü{Eñ{ÙAGNfsrqPKS 2357-318?ïúQ»ð—¾?7Wðan8?%<¯Í&¢?sÕ¥Ogá?Ai䝝?ä?4sãÉÏ??ïðAÓ×O?eRú$RÏ?"èö‰aóÈ?96Tzùº?]9#ÂM?cdåš–?ï®Lké]&?}9_ÔÈ5?WÞø'5	"?Zí9Ã2?qíÒñG?{iC9Šk!?ïùR6?,¤]W$Û?™Y:øÊË>ûþª{‡×?I3Œ­v'þ?+Ú­Öu¹×?ïô§Ç&<!?M5ïÆ¥4?32´ K;?%üÜ_?Qãéàãý?Ji¡÷Rø?ïÎEWøåZ?}–1ð`?:@|J?ND)—ú~?w;¯ãÅÓ-?{xÙÝåρ?ŽVM?'óã_0ø&?`2¢›Ì%ê?^ëaØK'?‹Ï³Áiëw?'Lÿ9"÷Í?ïì´y¢`ñ?LH-;Þ?-¹ïçå?ÛD3h·?aoçNšK'?Ka]¹J{AGN4FGL J2359.3+0215¿íóâ¯{ÈÀM<ÿdύÀ;b:	ç
À<´a‹·@ ëþ±Ì@`?ù·ãÑÌ?Ó˛ÿûMi?Û—ßÛq@ó‡œAÇ@ÏÅwÃÜ?ïÝH°rùó¿ïÿóÀ¬ƒ?ïÿ¤Á	¿×¾?kOÚ3¿àÞ¾fØ|¿æzD5ëAGNbcu1RXS J235916.9+021505?íéSPÊ?Íßíh=?qÏ¤0Õ?¶âw%rÎ?¶#ÃÇ0#á?ÌxH#×L?ï‡C¸ˆêl?nÌiåÚ?iW£¿ˆ!¿?tH×xb?‡Ù(Þm—?ˆpþn%9°?íLb‡ðµñ?§OÛö»|¦?jkhi
Æ?oe9?Âs?´ÉB?§<R7L ×?í–ëƒ5ÿ?'æ!»N¹?gbv@p×Ý?X%"(\eÀ?²3ÚÇ
?'ÆÓÚU7?î&mû07€?¼K€¶7£Ê?gÛè­Uɘ?u—…ãoS²?¬aÂS&b?»9öŽð¦Ï?îWÄ?¢iç̐ª?wʸ—?ˆCè)4.?œiˆö›'?žå¦×R‰P?ìwt^?¨äî,ž©?n''+½#\?qv÷Â|ü?»SwÌ?^:?¨ø(oZ·Ï?éÐJÒzûc?­*es1À?qô¨ŠUŠr?mŠYԕ¼?È//qÌdâ?­'"^
AGN4FGL J2359.3-2049?ž¹
=¿«ÀS"¾7ޓŸÀ:Z€U$õƒÀ<‹³¢,@U¼!É(@øУñâ0?·ç
¶<h¿›€ØúÏáÍ?ä6wÁ½o@8¶Ñ"¿Û¯©ü=RÇ¿æ‰RÄÈòM¿âR°Ü¬=á¿Ý¡z¹"œ¿Üß!c'Å¿ÞÎÙAzHÆAGNbll3FGL J2359.5-2052TXS 2356-210?ïÜG_?\Á»ÄZq?C"}¾ÓxM?0ÖÚ8g?oÛ?Ùð.?ZcEùJ5"?ïßO_¨uï?q3Šwæâ?9?ûBT?Cð§ùlK?mˆ ñÿ@¥?nu0zd~¾?ï‡õý?'Õ?sEÏYz]Õ?_…=5zi2?UP!R Ž_?ŠÙ
¦Et?qÑQ«i0ã?ïÁW°	?Z`#("ò?E!ÿMžò?,TDÁKo?|¯è)tx?Y";€Ì?ï°ôh‹ôY?qÄSé£}Œ?Wƶü¥I?FfՓ?€ÊI‡?p«À‹Ù©?ï ×™œ˜?ˆÑáÉ.Õ?KšEÖ «O?Z$qjûW?†uj¦—"?‡GlêÓ·¼?ï.
H¦6?€âg\¾Cˆ?jrQ\c5?bsWrNb?–þH«üƒÛ?~"ÉÙ´±?ïU'èAR?xm±Jnšß?\F c½]§?KO½­‹?"‹8õîBä?wÁ
¸AAGN4FGL J2359.9-3736?ïàËsöÀRºÛŸ'xÀ:òêÏS)À<ËR—|ˆè@8¦ÿ´?þ'5deÛ&?ÇrÀF׀?Т‰bñO@Ô×ãD8?ÿ‹O™Æ:7?ßð̆Uï÷?í\૦âW¿ÚdéÄTXG¿àJãq*¿éÓYG™ó¿×¸4½¤¼AGNbcu3FGL J0000.2-3738NVSS J000008-373819?ﻲ°cW
?q9¨^ؤY?cìÔJ‹¼§?[Yù™}×?x0=ÁË̦?iò¼²b½3?ï^rX%õ¢?•Õ¡*ß1?wXˆ!`¸?'þvýˆ7?Œ·%àS+:?ðdo?îýfa¢?'bɔW<1?‡ÿŸ"öÆ?ˆ´ÆKü?"Ã=BZâ\?…H7w²'?Šü·?}%l'DÖµ?UÀÏÜ?s-+ǒ¯?˜§œÏ¨ ?tO'ä<PK?ïT*œ‹¼a?‡Wö9—KB?€t»]‰²?v{"Ò¸Ó?Š€ÒÁáë?€CA¶=E.?î1K"Ù?±a¶!½?8PƚmO?Ÿ"ù ܧ2?¤ÏghÉ?ª:'QIê?î'EO{¤w?™‡Ë£Èj¿?—ª'h·tW?'¿+{8B'?¡¶aÑVIc?¦,´oÜý?íB•}o`?–7Í?Ç?žÐþÅV?ˆZ]qˆ?¬É?§eÖ?êÕ"èªAGN4FGL J0002.8+6217¿ÞÒ¼ó2_¿ª!gâE­À8Áœ©'žÀ;^`¯m@u@Ý®Éü¹@‰øÜö¼?®'‹`òË?Übþ<†n@%C1T??ü±åÃhÊð?Áºg"ôq¿Æ|Í[g¿á©c;8»¿çBëØ*Îá¿ïFMä¬g¿ïÿÌ~sM€PSRPSR3FGL J0002.6+6218PSR J0002+6216?j%Ú_P€H?P¯¦2?íV]6çȧ?°Ô¨"e?´{çvÚ‡?®Gõ6HGŠ?ˆLF{NÛ?‰ø_úF?èÅÔ¹2ïŸ?¸W/q‡¬²?Ëcè¹"²?¸(Ô¼X¬?‹%Uay?‡ñk½"Hó?íJg?²Ñ?£bàXœƒ—?²H"˜™/
?¡T'=<?*m…u:Œ?f½®ÝEä?êe™y…Ÿ^?Ÿ;Â÷y?ÅVóAUµ¿?Ÿ•ªÓ|	?`
z.#¼¹?UçWÇÄ?îD" ów?¡ñÀjFxh?ª½7äA?¡†Ó:Çs"?yý•Ç›î/?5¸L?é—'<
€?ÀÝ(è?ÈÓÍI@Þ?Àh¸P>?}¼B‹±N?u)ViM‰?í¤¸®Ý£Š?£iy'±?°þvh6^?¢…ÅJy*K?YuÛÁ2Ã?C¥Ò9"Š?ël§'»? ã<Õè7?ÂbÌþËÍ? SCXHPSR4FGL J0007.0+7303?î¼,wh}~@$ìaR*o?À5'c;8»2À:xM'Ðÿa@.!|Òc?ý¯Qvëè?€"'—s¤'?ÑøÁ²½W@QTeâXO?ú$¸÷WåÅ¿ I[=¾QŠ¿É)ùù€´ñ¿Øör¸"@l¿àÏ>šõ9¿êˆ6šÆÀC¿î³'#iPSRPSR3FGL J0007.0+7302PSR J0007+7303?J—BgËa?PîŒâ:k?î8ÂC±Û…?»gݬ:}w?¬	~¼›Ä?»c+ͨØ?ƒ4Ð
È*?«m¾ÌéY?Ks,.?·UtM³%Ø?žÓ®–Àq+?³ Ä. Wl?³`§FÁµ‹?¤:³ˆ—¹|?覩‹e_'?²Ð©ÕjÄß?õ/wšt?®]"&_{–==L¡¨.'$=kå	š<?ïÿk—­±?$Š}—ªÏc?ŽOù¶Ê?$Š}—ªÏc?Vß°‹?è?S[ᒀšu?îúýuÛÞ?°F†*F½Ž?Ÿ2VTЅÍ?°BÎÜn?{þobª?¦Ž/<µfI?î°fX_ή?½äÖCnÚ?¡—º«¾Þm?º«ÓOjBá?¨
ÿ÷5oè?¡…Æ8j?êjÄÜaï?³cä~ÍÃö?ÀQl"?ý
?®Sòô¾=%BAæ…=@éäJ(ð?ïû‰Pv:?Wáx%b?AÚ½†CC?Wáx%bPSR4FGL J0023.4+0920¿»,'È~	ÀJrÁÁÖυÀ9›íQx™À<0j÷ŞÛ@…K2Åz?þ+O¤ƒ¨?¼J/¼P?ݞ7@.@¼æ")Æ@½f'|F¿æ‡Y%5C¯¿»,y@ïņ¿Ý‹ßœ³)Ž¿èqÊÛ[¿ëbœ!´/È¿ïû¾½?'PSRPSR3FGL J0023.4+0923PSR J0023+0923?˧hW_ë×?ÃhLù
 ö?æ4"REÙ?ÈGRø¨üA?´/‹+¬Q
?®´ª=Â?ǦÐlr!¹?Ǘá¤Ê?æOŸ©9Zü?ȆҠ)k?¾5aáœgª?·eÁçö±¾?ÆòWÚÌ-¯?°¤°5•Í­?å ìFA?´ýXÝ)??‰÷
õÃ?©94*ß9§?Üò•Í‡?®'۝<iÒ?Ó·ä¼òS?¬¯z5ä?ά-Z*ã?¥¬š8ŒÃ?±|¹±^?«¥¨˜%€a?ëqGÅÞ¾?º­^G‰š?²ö±¸?¯¦çǜR?¶F.Z®@?·<Ô¿Š?éq`À蛓?Àîkkfˆÿ?¾.Ëxšª?µâ2¿û?µø±m+ð?£îÈé·?é%é5ä?°	/9	©%?ÀlOÐ^

?§Ì¬ƒ:¹?΁&µe@æ?«_çŸÑQ?Ù,xŠf‡?¶;«¦u?גôæ؉?²§ Y="FMIXED4FGL J0030.4+0451?ïú{¹YåÀLÎi­BÃÊÀ7‹…º¿"À;‡^@'7|@Vÿë]0³?ü"µ—&"?š¶‡øºm?ÜzRõñ@?þº{'pÖ@¸wù
îF¿­@}Ú²z¿»Æ¤i¬A¿ÛŸv¼Ï)¿çŠ©Üݼ¿ît‰u_(¿ïþQ>¶ôôPSRPSR3FGL J0030.4+0451PSR J0030+0451?o©t@	S"?©U¶Ú4?ï$zŠN'Í?ª@Þãí?—{€'Mcð?§Td0V4?›ˆ• ŸC
?©ª	¬»°&?í¥ í©Å?³ûâ®[S«?§á¦""
%?®Æ_°)?©åòÎï/Ü?¡	Åg¬?éâõ® ðY?±å›§p.Ø?Áú¬"
M%?°v`uäÆ>Ñg¨b}Ó2>֙f]á?ï½·E¦þ1?uªûýÎÇ?€™úè?u¨³ÔŠ†®?sG$Œøå?€ý¿QšÃ?ï,S§ê6·?§bdîÔúè?•£Áþ¢
Û?£›\Ty/ë?'ÆWmp?¡®úãbD×?íöt>Hî?·=;vÿ	?§µ¸iyZ?´!ãûH¨i?¡ðv'ØÛ?ž¬Éœøù?êƒ_w:Ž?´UĝG[Ü?Ávf0-Ò?±×Q^К>¶FÐÚ#¿%>É¥×¥…'ß?ïx(	«Ç¼?ŒuÜ(Ã?ú¥¯à5?Œ~ú1	nPSR4FGL J0034.3-0534¿—b£®Þ^ÌÀQ³g ù	À8™¸Øú¹À<øä@bFg'A?ÿÕGª¹|Ž?¥=mbÈÂ?ÍیÙÝ@%Û°_®¼A?ûåÛÏI(é?¤7ÈÄ)¿Ô5Ñ>B¿áõ6þ™Îs¿æ^92¿í=¶y¤0Ì¿ïþ×@ÄnPSRPSR3FGL J0034.3-0534PSR J0034-0534?·¶é}àë
?µmAs~,?焭I?ÉÁ)­šÏÇ?ÆÖó}vß?Â*
¥Z#?ÀÖ@WÎ?Ç©ÛÓrOË?é$aφn!?ÊF;vDA?¶¿ÏÖÜ?µLå½²É?ÎMðvòê?±•~KZRy?âòeì ­¨?´B
Zu[;?Åèx3Vu?¬©¯Œ+9B?¾x­¢†¹?¥1Á%÷ ã?æÿÇÈ£iÉ?±vH…Л?ÄĊW¡~?¦:ŒH?¤.u/¬ì?Ÿ‰éþTè?ê%…1q€æ?½Íw Ìv?Â^jî/?¸ÕlQKœí?±'ƒk•V?À<Œq×¢ƒ?ëÝ<AàÜ?Ưz"þ)3?µ–'³^WG?»©­Û<s›?ÈGBæؐ?°¦Ñ2ýh?ä,ýs!¤"?µMƒ²bÏi?ÇÇOŠVÜ?¬i֛H>Š?ªm-‡Ö?—r=áÝ^?çяê™;{?µCqPYœš?Ê5%	é| ?±üôÀñG7PSR4FGL J0101.1-6422?ímU&‰<æÀJ]c
'SÀ9nŸÀ<]
þÆD@3q¾‰=?ýút?¬î ‡—Æ?ÙÁ9d@+ß /µÐ1?ýMÌôåŗ?ïçlá)Ñ
¿Ï5¤&»V¿Ûò ›ìZ1¿ç"ò5<!ï¿ì«IúõÕ¿ïþó%&*6PSRPSR3FGL J0101.0-6422PSR J0101-6422?˜àR"¨?˜¥'tõ?썌û¦?ºH¼:F?µ ŽàÉ?·Fü<Ò?¦r9G8=?§w'eDœ?ìO ·Î—?µNIVÁS?²ƒÉßU½+?¯löòݯ?§Åó'ÖB?›ßßĹ<~?éÌA'g=s?®íR"Ufn?ÂÝ|÷'5a?«…Î` ©®?™ß
Zö4"?‡ñu>>«Â?í)‡B©ó¯?š$oãø?°<•ª£b?"§d®6{ë?¦ÁË;þ?¤‡Br1?ìĵ²»?¸ôõk²M?²u_`ÍE$?±ÞœZ£–q?Ÿ:¥úBTM?¦Yª6ç÷	?쇟÷à)?ºÄBO/èü?³ôVÄ%ìö?¶î×¾·C? "(±À{?—28Ê<rÏ?ë%½[ëŽ.?¬ÿtù?¾Ð"
&•Q?©e­ºÿ>?'Ìð*ïE´?ue.€[?ìöQZ]?¢e€UƒrÄ?µó×)o™?¡E&'y+5PSR4FGL J0102.8+4839?æ"U¢7½À,VÏ d#–À8ê0IsçXÀ;Óg'Æ~@Ý«PÑ(Ò@:Ì}?¬¼FÓà?Ðàâ"@"Ëê¡ô²?þ
þÙy•?ïƒÂwß5¿ÑØ)ø!¿ÝãJ<º¿âàe0¿ëÈ°ÞY½¿ïÿ¶Ï4†PSRPSR3FGL J0102.8+4840PSR J0102+4839?"HÅËäŠþ?•ªˆV¬S?î'mg%læ?©³AÊ'ó?™iM¶
K?¢Ik"R×?±¹«7Õf?¸ò~Ù!´?ë7ìßx]?½ŸøáÜ1!?´†íÎÝů?±ýѕ «?ÄIUã¦ø?®•µ$ã¯Õ?æø[(ù&%?²ˆö?¿ªzðê–ë?¦Å/ïbÍ?·76aHÁÑ?—uîÔŠ'?çlfì¯Q?£Ö°¶¢±?ÈJ³3ô'? ?/&õgj?ˆ Ü:[‹?ƒkçä'Ï?î¬?wuhž?žèñŒý'?ž'¢û$öp?˜'ƒ#+@Z?¢hž1ÖR7?¢ˆœPÈe?ì#v*?³Ê75E1?²J˜*ˆÞ™?°kT¥E_¶?²-@‰jÉä?§ÖmJáD?ê'1ïCø±?°
FèÜGË?¹I/û+–?£7
ÅPÜ°?ŸŒo1¬>?ƒyFÈÓLP?è9âïp]-?§KYĽ?Ù?Ë&æ\•Æ?¥ïÄäíPSR4FGL J0106.4+4855?ïdöEZÀ+½í6´ÈÀ8©Œœ[úÀ;áiF·G@h'"ß-?ü#iüóÜ?ª]é?IA?Ýg.!üT$@/&VÍl.ý?ó½ÿšT‰?ê]»Çí¿¿EQîµ)î¿Õ™ –ö¿àçÉÉã¿î"Yáó¥¿ïþ¥AÃnÕPSRPSR3FGL J0106.5+4855PSR J0106+4855?yA²°t…?g°uv¢:?ïq"`…âê?"½ÆM'T?‡Ç¡Z?e&›+\S?˜­9ž,1?¤‹œ'S?í2\¸?³Ë\Ô3?°AÑñ?^?±5«H.?šž' QY?—¶…7·Ò??ìÜȺ»Ë?©»±´|û§?¹9y2ÝÕ?¦+Zêš.?R:¯+¬ú?B9'é×ó?î¯cš	?ˆßÒ¦$´?¤wÿ'¬K‰?ˆ'œœ¥µ?~8ԁ§Ør?'êԐã­?ï\Ò|Ë=è?—âcŽ¶?‰®ö"‰è?'LÅ''fj?
¨Jm~·?•,{š;fD?íÀgë‡ß?±	¬	vâ?¬3q?×]?°0«Š A?"4³V};õ?'4v¿H,?ìö‰á¸
Å?¦šà:™­0?³>"êV?£¾Âc É?3üê]i°"?+-
ýÝ?î‰*•Í(µ?'•®ä•§ƒ?§E\ËDýÚ?'†"gNPSR4FGL J0205.7+6449?ÖCåCLl@¨Âa8ÿüÀ7n÷u³À;)®^L¼q@\íó@g™¼Õ?—Å
`¬?çQéßú@$wFˆz@ªIâøc¿­Èl뻥]¿à'5ÏŦ¿æ3ôÄb›¿èD¦ÃMÈ
¿ë~gä맃¿â²Áô+¶gPSRPSR3FGL J0205.5+6448PSR J0205+6449?í¡ƒ9þø?·Pë'õ:ž?•¸KJ&í?™LWO$Þå?«¦¸w;‡?²ôCmÅ?ØAG¸ÑBR?Õæ5áZÅÁ?ÖU|éàƒä?ÓââÌ)°?Ñi;]N9Ê?Îv–·^rô?éf³J<0ª?°œ?Ë5âª?¸¯ƒñfµ?¦ÎžÝFÕ?¼á¾Ý‡?©ÓJj\j?Ô¾' ?±ª 5MÁ^?à%ã'ü?²¦·‹ÞJ?Ç@2Ü1æ?£'¾<žéP?ëð¿š#'?¹¥±*
|?ªu×bEþ?ªŒ¥?j#4?³?}V4C?±LDžŒê×?ÉÃér±	?Ñ7s_ÚAf?݁ïr­á?Õиœ5¢œ?ÖõæÚY?ÑëAà}·?æ±rk'Z
?³fRF(@W?¿ÐÃHáèŠ?¬¼(J-
?ÅQÔ¯«e?®vË~è?¼cwÁz?¤ŸèÆl?åI؊´é?µ½ŠoÈn?̧™Kž˜?±w˒Gè7MIXED4FGL J0218.1+4232?ÒJ¼úº'À1"~"ÐÝÀ7Â>Nh‡À;aHt
@¿égã5@ô¸ÙÐÁN?Ø›À˜ê{?Çjþс½@)ÆP¤]B@á+'¿Ñÿ']<9¿ß-˜T<¿ä9‹!0Ò0¿çW_ã?€¿í$¯ÂzäM¿ïÿŸ‡ð#êPSRPSR3FGL J0218.1+4233PSR J0218+4232?×Ýã'p't?Æ©‰;R'r?Ò@.\e?Ëå@bç?Õáî}í'?Åz"ñ",r?Ä@_Q,?ɒ$FþŽˆ?è]HBÓÿ?ÌpîÓ¶?¶
?@r­?·™8åh"×?à–C¨B?µ :`»·?֒3Ȟ-Â?´á"Ì,½?À'‰Ð¬]õ?©'¸F0z—?°Ëay?˜l´ÍìK\?èáÞtj
5?§D4TžÒc?Äm QnÞ?¢ã%"Âô'?ˬxó ò?Á¾.R½€î?á$w{"í?ËEN~=G´?ÏÁ© Rä\?Á·®!ȹ?² 
Òh§?Àša'P±?ë'§¯S?Ⱦõ@*à?µO•™£¸S?¾Y*h´I?Ú³Ènï!?´Þ+QYñ?Ûpæ5î?·Clä?ĈX@UR?­J>q÷?"gÏêZô?"6š&?逯éDÛ/?°ø'_
®?ÇpF]¡4²?®-—qY@MIXED4FGL J0248.4+6021?ÏáÕZîk·?æ­Ü|m8èÀ8>°C)JÀ;
ïunA&@Íx¤¥Â@c]$žDú?°¯8½5Õû?áUÛ¿-ý¿@"ž9'û@¤»üoý"¿Ú\DNŽƒ¿Ú_
Q'™Ë¿â°£¡ZX;¿êuŒ\š5¿ð?ðPSRPSR3FGL J0248.5+6022PSR J0248+6021?ŒÝ¶©õ²I?¬Iž¸Þ?í²Þ°ò?À5ôn&y<?³¾¸{ËÂ%?º3[sªX?Ÿc‰}œ×Ê?°²=¦|÷?æÙh>õ<?Åk"!‡y?ÐV÷Eú¾«?ÃõÄCL—?¨¾ûwû*?Ï¹#=?þ?çU'ò±7ñ?¶Zk%Oá8?ÌyùWç"ò?µ©ÉÉÆç?•˜5!'$o?|ò°>Õ0|?è|ãX²ý!?«øÛØBÃ?ËYkùoºo?ª®fÎHÖf?˜uÖ4ÄF°?·
ÐvCZ?ëۉ/¶sf?Ä;^4''?»@òõ'£?ÀC,ғW®?ŠêƒxY"?Ÿ¢"aü4É?æÉëq†2½?ÊÝü‹s?єÕØ$ø?ÊKd‡>£?•t:ŠK%?'®§õ\Jõ?æú®ãB¹?ÀRñ¶Þp[?г_WBJí?À-ü¨ÄÀ?h'¨ {í®?Y(	ÍËÝ´?êgò¼æZ?±ƒ)û ?Åýîm[x!?±KO"ñ˜"PSR4FGL J0248.6+4230?í«Ï}i–À.£^·E|À;nµÀ@ÍÀ=%(H¦@S9›W3î@‹o"Ný?̓ÞC¢|?薈¢ÑPÀ@ˆšˆ¬âL?õ7xŠ*eÚ¿ïÿþR€ÖT?ïÿÿ>¹ú¿Ù¨ ½Ð/®¿áó¢Ÿ&ÌH¿ïÿwy´!¿î(zÝì¯ÁPSRPSR3FGL J0248.5+4232PSR J0248+4230?Ҝ"‰Ü|?Ȯ"Áq?á¬oöÄÍ?ËqB·Š›?Äûâ3D?Ãù,FSÞ?Ä]–îs×?ÄôÜèVt?è|ŸÒ(?Æ0¶97s?³dU$€°?°ÏþIÎS€?փÞo?0 ?³bô­@´^?Ûñ
kDéá?´äkpù?Ë(J÷Êý?±ž­_;?ÈëÏFy¶û?¥Èiðz?èÄ¡Þ?C•?¦ÀT'¤C? ¥ܸ»?ŽkLŤ'$?ÍUsÐÝ(?ÃÍÂ`b@g?ã÷|ìÃ?ä?É]ë: R?ÂÌ|Ù"#I?öûv¥Æ?¶–ƒºb?Âd·çê=?êÈ ÐT?ÄпڏÇÍ?³$vuíX?²Ç(…ö­?Êîœ&"Ú?±döû÷?♓Ƶ O?¹¾ßF]C?Ê«¼á®l?²ÄPmÔåb?¬ƒæÇ"R‹?•?âC+£È?íGŠûhŽ?Ÿ•"ÿmåµ?¡‡ ‡oV—?"ùà&&økPSR4FGL J0251.0+2605¿ïôÊùnÀ=~‹;26À:!["Ì´À<{¸;EPl@ÝgX(àõ?þ³°fd¸ç?×ɵÁ?äãkªs±@9à0Và@fw@(d"?íº@£^>z¿×÷½j.G¿Òn2b¨Á«¿æÜ>¯¾¿îú!~ÕÈõ¿ïû
ÝԇPSRPSR3FGL J0251.1+2603PSR J0251+26?µRž0_ÌÍ?µ\G©ã>?ëðó\zN?»"dÔÉy?¦KÚ	%?¥³"©Þ»?¶R'Ý—)»?³x¾K¸b?é΍:ÕWÐ?¹ý "p~~?»9KP$I?²ftÿsw£?ÁFC0V_?©|"ÿàt?ç{˳L'?±lü؃9[?Àʎ8n±?¨×=Ö.³7?Èëâ´.?£<@j?ãÑã#È©t?­ÿ ÷–V?Ç̐¾öíª?£beÃÚÁ?¥€†Ã!T?¤\¨†ù,G?íCxHÍ4?±žgìÝÀ8?¦Huèùùã?¤ªårY;?ª»v¬7^š?«$ØOØs?êáÆHp©ƒ?»qFqÜï¸?»"d9C ?¶'÷[_¯å?°ùΌ»EÙ?Ÿ©ç—Ý?ê@­½›Š?®²xí	Ç?½Ō'–?§µ§'ç´ì?°=ø°–»b?"è܏½?楺cd?±²;êk©?ÍLü¿Ñ=?¯²ÔÎEjPSR4FGL J0307.8+7443?ï3´.è˜@,p&grÕàÀ8Ûö"o³íÀ<Gö-fÿ@aßÀšdp@ã!ž¶9?§ãÐÊ][Ñ?ã¾]~
qô@1õÜy@àTÍâ?Ò®íÞë2i?Õgá:Âõ¿Ö"ÛÅc!¿æ_f¿ï¯âjmÝ¿ïÿÞ§À£ÊPSRPSR3FGL J0308.0+7442PSR J0307+7443?oUq8´Í?'üA¶0?ï¿?š?'ÐΒ‰?pµó÷›óà?ƒúÆ+/E?"4w¹D?'ä ´'$â?íó{c´Á?°X››©?«Ê[/0@?®¡cb\ì?¢†72–?š'ŸîL˜?íO=Þe"?£ñDZµÉŸ?­×…ëð\'?Ÿ<îÑbt?E׈wè*?8(Ì:Ž´6?ïÃÆ*
.q?m@Vp?{b44@¡?m}ŠÀï?ilçÕ~܆?sÌ¢"9ï?ïÅêO6ˆ?"åè4ƒÖ"?pTdx&	°?zH¹­h?ƒí³É±êg?žU!vp•V?îä‹@¡—?µÓJ2ô·?©6J\ ó?³¼©[¤=?'p>Ò.Ó«?'kŒ»Æ²Z?íåÙb Jg?ŸLl=‹"×?¨jJs,!»?›ˆoÁ')?¢é€þVÇ?Ž­äÝßn?ïÉÓÁÇ ?læSö"þ?z§"ëÏXX?lÞU¶?íPSR4FGL J0312.1-0921¿ï®:6Ì^­ÀJ/]$žDúÀ9ù…¤ðñÀ<ýdDM@JXE;st?ýίá»v?¾¿<ÁQnˆ?ãª)Ÿ5ºÍ@!»/fÊ@>Ï5ݲx¿ïÿÿÊPË?ïÿÿÊPË¿×,åÜhKC¿æÊ{ÿÒs¿ï*Aò闿ïÿö$´ë/PSRpsr3FGL J0312.1-0921PSR J0312-09? OϧÚ½?¤ã[+5=?î?¯mkh?¯t"Ê©…@?œXj»×‡?¥±U¼¹Èþ?³lÚC¹Û\?´JÔÃ÷{?êmå¥z'1?º–vRÜ_¬?¹#ø•¬?±ÓQÊ?ÀCh"¶Ð?«ü¤:cQ?炊׽tH?²zRuér<?Á²løx?©~!fÔç?Í9è0LñB?«ß©ªP#™?ä¹|¸ã6?±Œ¤c0æ?Â_1ÞõCd?¡ÎrЊ¥?žL¹Û!?žÃµ´Ý\?íÿ‰Ð£Æï?°C½‡N? áhŠ}?¨Øj¹Ø	‰?¤èmmÖ{?¦Þ
^i?ë¦Ñía܃?½r3_d$Ô?¸U:qþª?¹ãƒe®8@?±ño:Í?£a'­O?éµw£·?°_Øß'?À1iÖ·?«2mž?·Ð¹Æ‰? nԌX?ç>,à֐?³¨w?€G?Ç?ûrý?®±IMv·PSR4FGL J0318.2+0254¿éÂD6vð³ÀEË]9–ûÀ9ËɪiÀ<yÿ–M´¿@Ÿh#ÕÈ@lŸÞW8Ì?·Ô=À'o?â">¾°@ ã§Ú¤ý@–ÝàE{¿åC%ÿ˜üç¿Ç×±j¿×Ïxäl-¿äË»À5Ö¿ïÿúÁҝǿïÿÿ" 5•PSRPSR3FGL J0318.1+0252PSR J0318+0253?Ÿs'–ŽE?¢Õ²ÕxïŠ?îæ¼î;(?¤0HüE]?m¦ý0•?sñ¬¡ÒW?³wa.,Þç?µA‡ˆ¡'?ê·nëg?»/k}|'ˆ?¶ÐC[SË ?®l"öµ¯?¸£7"oR?¦¬>Û+?êTÒì1Ó?­êF
.Ö?µFÅg¹ÞÅ?¢‰oŽ"w?Ðþ>DÂc?¬'"ãZ
–?ã6Ú@9U?¯1ÀÁvŽo?Á(ޒ5ç?£%uì|{¸?˜1¡È0n?¤>~£›'q?ï_€T_d?¥
ñºÞ¬?q‰¸–ƒv?q4í欀ª?¥Ó ´<ž?«.™ݓŸ?ëpÑ#s£?º¿Bð8?¸û¦ø8?µ‡¹SÓy«?¡§?ÿ²B×?˜6$ь0?ì'æ‹©…º?¥vrÙ(Š??²+¢Ú°Ç? ¦Ó¬Ï|6?³çÐq7žÔ?œì}j"›??è˜L…úD?²ñ¹Ý?êç¦(."?°.ËTޛÛPSR4FGL J0340.3+4130¿ï¢`–SûÀ&%kÊSvÀ8ªµr£ŒÀ;ö5©/8Ó@šV=#vþ?ûVAU4æ?§ÿ	µáMã?Û¨Ÿ{°Ðm@/ŽŽ}Ü¥?øŠi
/®Ä?ï¶úÀoÇ?–ôu=å¿Ì?€Êë¡¿àÔÀŒ!·¿ëÙ-ފf¿ðPSRPSR3FGL J0340.3+4130PSR J0340+4130?d
9u`?e''{Ìí?î䀫1?¤+g¿{? w#ïe¬l?£z6Ýú¬
?—1ªÎÉqç?¦ãPztmï?ì EÍ6 ›?µþ®BkÖ?µ1fãæy.?³ëǟŠv?—ž^`™®ù?"uêSJžÂ?êõ²M‰d‡?­k4(?Á5jýÇ8?¬¯TDd"?^-§@ÀÌN?OXe©>«Ä?î
Š~ý?"BT%€žõ?®mZ ‡ßÞ?"æÞ¾3NX?l±Å`f?ktB'…ë"?î¥{—‰?¦[úÂGp?£Ý*=_8?¥Gfã7=?‰QÙ-ܛÈ?'w¬l¬'ô?ìàqâ<íé?·I³­`Ç?µÒ5ÊË9?·iü¿uú˜?ˆìdÐ?Šê'.1Û^?ìGд…P?¨ŒÒÀ9"
?º©ç*Ø,
?¨7aäH)ê?A²1óç?9³––Œ£?í®ß¾÷¥? !¾®¶h?²e­iI	?€Ï¡íPSR4FGL J0357.8+3204?êYÿ>[¡À0{ÃŽÀ7qJEžpÀ;…¸èz0@Oð}+#ð?ÿÜЅ¾ñB?š"éß,Jâ?â{+ðHÒØ@B~ÉÀ¨Ò@ÉD"'Ô0?¢Žmìl¥E¿Ê¾Iý$-‡¿ã#³In¿ìXœ¿úÙ¿ï»x¡§Z"¿ïÔ+Á#÷+PSRPSR3FGL J0357.9+3206PSR J0357+3205?s¿A‹Fâ?/ÛíSŽs?ï†qñVf`?ü™^¯d'?"ƒâØdÌ?†ú5)œJ?‹±–£`æ?¥Œ'Tmï?îÃǜâ#?­I%O$=h?™Ä;¿ÚÝ?¢ú;Úq‡?¸Ï5°™˜ö?¦''XA<?êMµ«{¡ê?­õè6ü°?´Ãó‰W¶?¤¸{p´>–{ïSwÕT> v|§GÌ#?ïïÊ0mä"?[·ÿ[ÐkT?`5¦0Ï(?[·P¼k»?xƒáX@z?|Ÿ´WÒÑ?ïc<»Ð®·?'ÁÈοb?ŠîàmÊ{?‹&fˆV?ƒ˜"樦?œ©s$'?ïKє÷?§¼òÄkø?'jU;ú4Ã?¡ã€"ª??²:À( Eö?¢}cs¥?ë"h}?­W]ÓÓxÏ?µ8¤•@Üy?¦!±/>r±F'UÐv>ŠÒ¾Ëú£¢?ïኲBï?p­g2Á·?nuÙ9T¼?p­W"ÕËýPSR4FGL J0359.4+5414¿êǍÄèì'?ìR«~H…UÀ8¢xíÀ;€k©œF@۔œê@öß$¾%j?¯!ÇÐ䉂?Ý»Ÿíp±@'"M‹¤
'?ø…ê ²?Ö×Yƒ)Ì?äêÞÐÛOG¿àá@!X?¿æx'vµi¿ïDJ¢Ž-¿ïÿü9¡â=PSRPSR3FGL J0359.5+5413PSR J0359+5414?"¥Ôkr?°Ç¥˜ƒÙ?í®Ü˜¶‰ƒ?¶WZ¡¾y?¯èÁmD½N?­…Ù7-,£?ƒaæK7Y³?¡|'º¼°É?éàÓL˜#?·¨ï¸_,‹?ÇF•Zð'x?·ARó§]ü?†Mñƍ?ƒí0{è¬?í4—O"?£:GG¾æ?³'‡Oµ·í?¡2øx<˺?U;
`Ôï?@W}!(?îvyÏ­Zt?Œ+/]ډu?§îŠ¯t?ŒN½ðit?0 ì%*ý?ºþ¢:…•‰?î*Â;Ö?¼0Ý>EFA?¥F#e_Ö)?¥ÚöiÕæå?p‰<=>Ã?y" `"¢"?êáû!ÙÇ?¿¿dPÙÚ?Ãóəo/ì?¾ÓöH‡¦?|ÁeP"Õ~?xaì }š?í‹C2¸A®?¢ókû•|?±ÙÐ]ƒw?¢àˆ"¯<?+Ýxåó¦?y¼²Š/?ºÅkã?_5aå?£úÆÝ®ù&?WãBY•PSR4FGL J0437.2-4715¿Þ¡CØ®´ÀDû† ˜'\À8Ǽ_—?LÀ<F…½CÃ@¿bå¨eå@lBHyì?¨žÕ˜£O{?à™ä½¯M‹@1ђً÷ð@Cå²÷º?ÂÉ·Ùö€û¿Ô$¼øÄL¿ãþ´;Œ¿í^•a¦Ž¿ïÿØ'sâP¿ïó?B5.¶PSRPSR3FGL J0437.2-4713PSR J0437-4715?'+R†¦?•—ó(
ž?î_A¡Šÿ£?¯·PéY"?¡v_¾è™Ã?§@Z?êæ8?Ÿ' Ö?¡Í"èé€:?쥝gž8ª?³¦g¥Êk?³p9½ªµ?° _q}ç?º¼ÅÌ0"e?§fpæú?éP{ôJȯ?°µÛ4ª½¿?º¿Z'y˜%?§•""$˜?iGŠÕœÚ5?^r5C-"4?ïURË\"?‰)& |?œŒdNt‡Z?ˆÜ?‰»0y6Ñ?Œ§°}¬–?îxçM	•?«¸µ¢¾?¢»ðQNa?¦$褑Ö?"v-EíÑÓ?–µ¶';O¯?ìzÛÒ4{ï?¿•ýéál?·–Å?¾mû}†µß?¸o;JyŽ?ªTÿ ÷?éß*¹Ö¿¯?±j"£¤ý~?¸û:õ#¡þ?¦?"Ì%
?IÑ42æš?DctÝ9?îܐ¾}K?'I¸ZÏÚH?¡ÏºÓP¦?'ÙK—JbPSR4FGL J0506.1+5028?åj­Ì'¦q@îcŠ	À:ÚD«*»•À<ÝR‹¾@ œKZÇ?þá='AŽ@?ÏÍseÓC‰?ïmß«÷@H±il«@"0ðÇ(?â
—Íç¿à¥Ã=×Ñä¿ÔÄAéã?µ¤Va
±à¿ìmc`!¨Ç¿ïÿ°_ïÉPSRpsrPSR J0506+50?·"úL` "?¶öt>ôÏ?éwÏfÒi?ÃB¹-]±6?»G8×? ?¶k%¦£Zr?´ÖÅB@¡™?»0µ:½t?â·[FÛ~?ÉPÐk׃N?Õ[˜"=3_?År—EÆ!§?Ñ £<õC?°ª>tB€?âµ¾¨Ç´à?´6ç¨Îz?Ã'ÄgAû?©®§TºŽÔ?Ì¥\8˜«f?³¾™IŸ?åBÀ
‹c?»qà!Ø?¼ŸG6(
Ä?©ú¯óýõ?¶vFgÊ=?±™<ô\pµ?è‡'Ü4k9?ÀmD7M°H?ÂØ%l1g½?¸Æù–\ã?ŽýÖ§c~?§ò	T41?äÞÖÏ|vë?̓¢ÅÎg?Ôibƒœ›ñ?ÊÌH"D#?Éi»…|¬#?®²¢šÖž?ä¯.§ïXú?´VÉû·
?ÃىÜë±r?«±ð–j5	?¨!t)S¨¢?£NˆJÓ*?êô#wm8¬?¼ËGs~tG?¼N*/~rÍ?µêeê䑚PSR4FGL J0514.6-4408¿Ð?ÔR
z"ÀA´^=¢ø¾À9ôËbi¤À<EÌòŒyö@Õ÷É$̓@X2%ìù"?¹R"¡?èԜ9‡
K@#W>«6z?ûÝr~øƒŠ?ïëý^åé~¿Ï͍çߢ½¿æhþ0Q׿ð?ð¿ïÿð ¼x—PSRPSR3FGL J0514.6-4406PSR J0514-4407?½ P<$ì?½?dëxDÆ?éôÎÛ½"?ÃnUS?³8øÔÜs…?³|H"â
Õ?é®hpÈB?Ñê"ÆžO?¸:¥Zêrª?È-õµèôe?ºR½pÊ?Æn–#?܃t;µM?´A'Dsgû?Ù7þTëP?³F6ފû¡?ĉàõc?©ŸójªË?ç8«
Þ?»U°Ð[¼X?¦MZ_s¸F?£²_Ctƒf?͉ý5['´?¸[«YWº?ȍúýÀ=P?Ã[Ãñý´?åÕ9û?Ê'–H‰å?À"S¾C?ºýØÈÙx,?âs³>cñu?×s©¬?Ò尛5G'?ÕÚQ¯þ"?ÀeÑЫ)?ÁÌ M%?Þ,þ咅B?µ#']=¦\?Ö2{ʞÍ?³‰‹×Ս'?ÇA
ŸžÉã?«Ã8ÉÆ?ӇÊx£nž?ÃÑê\Äjí?Àô i¾é?Å¡a?áÿ©>Áö?ǽî!o3MIXED4FGL J0533.8+6800?îû#	DwS@2/À~à°¯À9j1ZëÞáÀ<`qªm@YZô˜B×?ý¢"#æ?²q¬?¹~f?×áäù~@#ûb(E@ÒÿZh¬<?ï½(êÚÔÍ¿ÓßZÃðÛ¿Õ³Üȃ<¿àŸÔçM"¿ì4 ñ|¯¿ïþ SPSRPSR3FGL J0534.0+6759PSR J0533+6759?ŸQ^5x.{?œ1ªËYÕë?î¶iœYp?¡­ýÄZp6?ƒÂÜm…'Ç?…D¥Ø^~Ð?®ßæòø7?±6ŽŠnnÎ?ë(ԕ̎?»
ð´]•1?·¯k_Ùá1?°ÒÚçÜ?·¶¼a$,?¥4Þ¬?éçû'Óë‹?­5ìÅvÞ?¹	g‰ôWx?¤oIT€âs?È
DÒlôË?§2m5n"?ç<û!ã™?¨6"	
™?·iŽ"ª®œ?•ÐB…Þ?§˜Qڎ
?¡©'5&e`?îc`«&?¤ï=Yå•?Šhƛî?…-V2?¢>5C#ƒL?±cì´TÎ?ìBÅ`X§?¿³sÂ;ñ•?´Êº\‰x!?¶>=JµÇ'?¨½b§ˆ|?žºðsžqë?ëÅ߉מ|?©³þ3]©?µrR©`å?£íÿÈ-Èé?²4^Щ?˜}N˜?ê'¥ü Ç?¥ ¬‡'ÌÁ?½‰>ºrNž?ávåÖVPSR4FGL J0534.5+2200¿æhfë5\rÀ ž³´ÎÀ4^ZXTÀ8u~¤˜Ñ@q?%3@¬À½ÊÑ?'
æÒ(ú?Êʖý'<@@ñ«!Z@GP÷iY¿É§•ßbÒ¿ÝÁíz—¿ãÑÖ!	e¿åÛ£>Þâú¿êô~ø-£§¿ïÿÛ¸"ÝPSRPSR3FGL J0534.5+2201PSR J0534+2200? ©ñ÷%Q?¦ƒ´¶ó 
?زa`1ø?ÐÐýóO1Z?âœ=ÀÕȟ?кÕ3Mµ@?"wwÍðLÿ?³Ž:c'ÇN?í@`êj[W?ÁE®_ú<?±·yD?»‰©?Ñ9èµq͉?³ú£N€?ÒhbâDÑ?´N%"†±?Ü©®ç«í§?¸²«h—ü³>ªt@q"Sp>­p¨ñ˜ª?ç(dföž?À‹k§²¦?Ñï«éH[?À‹‹ÍV`?®ƒE Cã?¢\EÖAù?ãOÒ¦*¢?Ðz…¶Ò~V?Øx&F)Ÿ?Ðr.yBÀ?†h¸]üuâ?§Æjñ±Ø?흦!Îm?Â؟FŠ?°E·å_ã?À1*q—?Î%(?'?µ»©£wÊÚ?ӟڗKò®?ºUãiúÎ?ÝR'Ô®m'?ºOÄA§>¹—_¶£š>"Ÿª'ñÎ-?äHcø^1J?Çx2Z‰þ
?×o7‡»1?Çx1Ù°¤½MIXED4FGL J0540.3-6920¿ïÃëóa>½À?€¦—®ÞÀ8Pè¬&dÀ;1u§L	Ä@¸Ttvt@õV#"Cø?¥²žù)ø?ÔÆöôév@ ⟜èÙ@µ¬;ç%?îu×Ra̤¿änìF嗟¿ç	#•0~M¿çñbXdÆ¿ì6§â1¹¿î¤ZÝò%PSRPSRPSR J0540-6919?⓲é-½?Ä^Bm/OÆ?ÀTÀüÛ?Àþ+áҏÒ?Ñq†*&?ÀuÒ_?½0Jó:Â?»²í<˜?èÁK]ký?Á©öòÿÖ?¼Å"2!eU?µZá%ˆöj?Þ/ÇU6	Ê?²0p@ßã
?ÑOSÚó?±ˆÛrXð?ЀäÏÖu ?°__hɬ­?Á¶Ë‡í
¤?šŸ@é×?݃Ž´}?¬,P-#€Œ?Ù¡‡Œj¡?©'΢GY?Ò£z5Œ?ÁMPB(Ñ?Õ«Î0`V=?Æ0Q%%m<?×°"Ujž7?Â>šDQ?°ç–%ž?³"Ä[ Jõ?êY¥_óŸ?À¹ëYæâ^?½%ëêýÂí?¸`3YdCx?ÖÒ°ª4úç?³¸W{–?Ô^
ínØÑ?³Ã¯Ìè¥?ÔÏDh\,H?³`ß_hÉ­?£hÅOû¡ê?ƒÊp»¤½V?áÊ΋Ïèœ?±ÌX¬Á?ÙýJ>ή
?±1ÇÆE1MIXED4FGL J0554.1+3107¿ïÿ¹ÛÐÃ@±@ìFÀ8²¥xÊìùÀ;êʉüm¤@Áj‹@êPÖ²(Ý?­áÀ,ˆþ?â+`kz¢^@+ýxÄ6ü?û£Z'"ÂÀ?ƒ¢=×üÖ«¿À.²šò_.¿ÝôÌÆÐ&¿éÞÿQš¿ïÿþBe«+?È^9Tš6PSRPSR3FGL J0554.1+3104PSR J0554+3107?_Å_2±S?h•õî}?îfÀ'Æ…z?¯™G†ž·ˆ?¨•ÎY¥ôØ?¯˜Õ{&z?ƒ4àÿ¬"?–Ä|ʕŠÍ?ê°Ïâg$
?¾²Ï±¿¼T?Ä	rfòã?¾™
 °ç?Xß?•%¹¾v?êkÅNm?°n›`þyk?¨•Ü†åH?­Íè~úžý?_wÈ°~?N¶úDKÎ÷?îä9ù1@?‰À—6žë? Åˆ£¼­ý?‰(ÏêÔî±?^Žc¶Uãr?`§wêþ7?䲔	?£ø¸ú72)?¤ þš}®Ò?£e`‹hÐå?}Z\ñ1Uï?—ÔQç®n?êÞ/Û1`í?ÃU"Ü£Úe?Üm«Ìnz?Ã#û"ܵ?"ÁKu…y?Œ;Ö
öà2?ëÛÎÜO)?©ÍJ;±ˆ®?¼e':‹¨P?§Øhóoµ?2$è¯Þúú?'áè¸y'"?ï(f"!?Œ¥œ'
S(?ŸÇH§¯I?Œ‹9C¸ÅPSR4FGL J0605.1+3757¿Ä˜ÜÒ¡@ 
ˆ~¿#À9ÃÕ>ì¥À<'	µól@5&ƒwnL@ÖEüc"?»×²?>Ÿ?è¬kbNª@#ú<B¦m½@ý©¾Õ¾8¿ê§¼r¶?ï쎞"Ô^¿ÑU+@ªÀ¿æthAÝÅî¿ï{û#!m8?·!¶‰PSRPSR3FGL J0605.0+3756PSR J0605+3757?g­W*~˜?n3ßÎ*ə?ïŸ^vq»?‡Ê£QÔ3?'=ŽÐ[+?ƒÖôú+•[?\±ÈÉn?²÷Â~´Ñ?ìPݯŒäÄ?¹¥ÀªÈ÷?¶!æ"çƒ?²¯¦Ò5n+?³[qËt]?£EÛS
É5?뒻o
"?©Q¥eßë©?°²½}>?œÀ³{ýXY?¢^·gØ?†]
…°@?íû<¼Hñ?h_ÏnHÐ?œh©PD1?‡ò"l?sÁãq/?nÝj¡*ÿÕ?ïv}¶Ë>é?Šü%…³c?ˆ€[¢
?†kw×®Ñ?'1‹ÿ'J«?¥÷_Ò¶aJ?ì"|ì™=?¼ÄøÉf!?·O¸wpÈí?ºn²‡ž'È? sSÐ/Ún?"Nêpbì?íbºVË? ë­é€äK?®›F¾má?˜/qMCVv?z<~¨ªî&?e"$ÀY	?îøÙ'è¨ ?Œø+÷ßÞ?šU¯ûSõ€?‹NÓÃN-fPSR4FGL J0610.2-2100?š#Ƙ 
À2.8ÅCÀ9¶òÔô¹À<cÅü-ã@LÏõv9B?ÿÍø`ÏM±?¶žÕ)g­?àB««êÔö@"%p£×
=?æ'rhÓ(1?ïû®Þ¿×UÌeHÚ¿Ý+'€Íoà¿æš._8õ•¿ïÿèM[Óe?è:Î*šÞPSRPSR3FGL J0610.2-2059PSR J0610-2100?°Œ"Õ«à?¸OMŽžÖÕ?ìp±º2ýj?½—
¸¥M'?§Û¼µÅ¢¡?¬ÓÑÄplV?­Ú¿Éò?µ¶_ˆÊÁ?ëÐQs‡ƒ?¼ékd¹#^?²ïV­Ù?³~ëQùñ?³LcÏÀïŠ?£l†XL±Ú?灚c1íR?²ýY'^[Ù?ÈSd‹ÅÆs?°''PÇe&?¢Þï.ä~?ˆOÍåe?ëÅò"FÑÌ?¢†ªïü?¸ÊuVe?D°WLø>?µ_š|§ø*?¿KŸ¡×'Þ?ë¤ ×Í1?Á"fö?s?ªþ½‡Jç¤?ªþ~Ü»¡?ž¿šÄ˜Ê?¥ÎÂí¼5Å?ìÖ}Ü_øõ?¹ùÌ'w?±œ*m#àS?µ¢ƒÞÀkö?¦aª ò¶8?š›û_%?è½GãîÊ?´4ó!¬?g?Çry ¶Œ?³FYÐÍ?}›U?p[Sø…O?ìVÛ² ³?§Fèã'?»îLÏ<?¦´òùMPSR4FGL J0613.7-0201¿ïïA¸X2À"œ-IfËÀ7ÿ6)‡¸ÇÀ;…ë¾íç@¢fè¾Æ@#¹…È+}? Ñê¡|šŽ?ҁÝ$Þ±§@/Qߗª¬?÷ÚöE¿Â1êžCøR¿Ôœ¼C'¦á¿áTaì""9¿å8@Ž:–¿ï
žT}‹¿ïþ{›Ñ&PSRPSR3FGL J0613.8-0201PSR J0613-0200?cÍ"ôf?dǪˆÞ4?èç…	ꏀ?Â#L˵ ‹?Ì·Pvm?Â)ý2#?'ž©ßô,?ŸZyõÄ¥§?ëNÅÑ8Ÿâ?º&™zmŒÿ?À'2?ºO÷,Oqá?œ¯á‰¼9©?•"q>[°U?éÏûTìã»?°m~}ßSã?Å*z¦ö`?°ö+æ™Å?ZmȀšî¦?Mu19"?íµ¾¬‰Ç{?˜a÷±ý¿?±èSyWbp?˜	¨·F?e		"Unf?`éÿ2?èò?^Jõ-?Â}	e?ËâÞb‡šÐ?Âf-
æ"?…£tŸö;A?"¤;¼¢:Û?ë†Î"ä´?Áùý‡€?ÀŠSí	{?ÀÁÊBâ[]?ˆáÈm¿?ˆø`j)é?êÆ$"™­;?°Ÿhh-¯?ÃYQl¦"Ê?°/¢/ðQš?<Á©^{?2%]Èô¾Ó?íbÀý5Ë>? ÷l
¾[O?´ÍãVF˦? êøîÕ…PSR4FGL J0614.1-3329¿Ånû¢ð|ÍÀ5Óä öñÀ6åʅʯ¼À;7Äe>Š@æ]êÁÕM?ùkâqy¿ß?Ç+?ÉÅ?ÒÅq"tI@Db0<î?û‡"»c¿ø¸°W™¿§¶™bDÌ@¿ÕoiÚº M¿àz4CÔk'¿êD_½Õ¹¿î>¾L‰"PSRPSR3FGL J0614.1-3329PSR J0614-3329?{Þ¾2öbu?€ÄœpœFÞ?î¤ÞS²Úˆ?°åžHã›1?¢6C"(?°_IT?"@Hìï1E?ªGþ€ÕÒ?îƒXƒ5h?±ƒŠ"½?œT¦£×ÛÖ?¤àCËÂó?À͘ó?©Ì='ªŸ?åê{ÊÓñ?³ÃœE/.ù?Lj{{ý&?®,
#a²>s,¥'ä÷>'Ø~Øípá?ïݜ¤w)h?oà&÷Fc?q1š¡hZ[?oßõTõŠ?ƒ½ÕnT?†[ïͪX´?îÉêpL?²ýyÎ.>?ªSúe!Çð?°Ôèå?'ÿð%ˆ?šEñ‰—.`?îõ'o(¬Ç?¯†ã^'?—ÍÚÿË?«Žó:"<9?¸Ä	YWûŽ?«"~ÏG?æÔE7JL³?·Àþ"±Wš?ÈLæuóÕ®?²Ü†ë¹nn>bÎtoîÆ> !@m·?ï‹+홠û?"úr¹8¤?4ÿãã±?"ú
fõ÷PSR4FGL J0621.2+2512?̼÷dQí@L–F(~À:õ۹ϚÀ<'¡Îò@û@ˆuZ 	 @mYO&®À?ÇéKó?ïÿÂWþė@ öHÇ@±B%¿â1؊p0ë?ìœÏCŸ'?¸¸Û¾­$f¿ÝèŠBŽšã¿ïìü‡7¿éL"b¥¼"PSRPSR3FGL J0621.0+2514PSR J0621+2514?'¼îm?"DZÙ݄ë?íYdÍC?¹.¥´‹á–?¯éc›Û¾,?¶ÄKc1¦â?Ž…8)5Z4?œ½mU»?Ô?êHÀ|Ç?ÁvZlˆ?Äô¬x!,~?À?%&L'L?½á¶zE?¤‰Ÿƒ@üD?ç'ï*'?±z²PY:­?Ã{ƒh±ì?«l>28ä?š~?dޕ¼?ÍÅ ?íùÈ¥Ã
?"èÆ?¤a?£$UíïÈ?PÌMçU?'?ž¼É="?'íôÐüü"?ì
¸Ñ&?À•7`?»â'Ië?¼õIÇãóŸ?€ZmñÒ?‰UT9Jöà?êhé-ß?Đ%D»¤d?ÅV¹à‹ñe?ÄâC¬}!?¯þ)qU'5?›äèd'W¯?éHĽtÑ?¯o¯–TA€?ÂÝe…Yµm?«Ü'Dn@'?tκ‡Ø«m?ef'ÆoÈ0?îå:º0­?'˜S7Nd¬?ž%O'Œ?`teÖ¿,PSR4FGL J0622.2+3749?ïôS'ç@%òµÖ\À8ÍIï7ZàÀ:¯ç¯§"@ìáÖõÈ@E!Whœ¢?±qta{Æ?êQ\1Y@1p æ)•%@þ¢vb?ÛÛPޔËT¿Ð*~CQäN¿ã¤©,´"ñ¿î€úfc¿ïÿîÝÃÀ	?ïrbS—WPSRPSR3FGL J0622.2+3747PSR J0622+3749?Œ'*•"w'?•×é ð"p?ëûg<O;§?Õ0˜BŽ?¼"€ÉÅâ?Â/Aݬ)O?¢Ivê#<?»¯ÔL%¦
?ëêá÷Ɔ?Ç$x'/di?·"d6a-?Á'`ˆ^'c?²£O҅†X?¡ÆD¦Wâ?çB·7íµ®?±×Â;Îï?É£{5¼‹?®ŸÝfë?3ÎÍ8;Ù?+¢Ââ^Ä?ëQ>©ˆúæ?­ËgÙïOM?±vðwKç?­Á7mT—1?–êB@¦À?¥ûî±ûš~?ìv6›¦?Áòbˆ‹T\?¶"º–ñ?¾0áòæ?¼(ô`¨?ªÅU;&Z?캃zà"?Dh19*?¶tdŽ.ˆR?À¦@'7c€?¥w½¨vê?šÛóë¦ý?éC8v¾ù%?±}ߜ泱?ŕ.»TTk?°'óœü;>÷.Ø¡†e>ù–(qË`Ç?ìE	Ž8f?²Õ-øV€z?½Ö@ Ñhµ?²ÔRú¢PSR4FGL J0631.5+1036?´nËÔ?Ý`IôÀ83¦AGÈìÀ;qc´~ë@[áþ@и,+Ø?©%œq».?Ø 1ί%@+"ê»Ë?üg¿	ў?³½ŸˆF
%¿Çdëýi¢±¿ÙdÛ·K[H¿á~®üØ-S¿î œ˜Q›¿ïû¨¸Ž!PSRPSR3FGL J0631.5+1036PSR J0631+1036?iŠ+ lív?käå·p?f?íÒ4•³Ü?¶ÄGÔ;<R?¶ä"÷?¶$ÚHE?ƒèÎȶ?ŠÜ¨ôÄ°?êF1•x^?³Ø/ZbVt?Ũ®¨}Ü?´	Êë1x?ÁûŠèõ?a&ÀÆö?ìýi¦s?¤/"‰wÃ?³ä3év¸?¢A5×Êe?aë'S·ß–?M.^"æ
?íøMiÈÏ?Žõ1%Ã?¯\p?wg?çÝÈìš?y³7ÃòN?|
½j[?ìšïàÖ¢—?¹ï²çÀæ?¹–ÅÄÑÈã?¸¥ª	Œá?uƒÌä+Üz?}´‹Ï,?êòÁÐ3My?º,ïPŸ£?ÈÚY¨<õ?ºu×Ù¬j?'h*Ð$þ?Â…½O?í'¯ùò?£dÕ~¸që?±5Õx¥ªµ?¢!^ÙÛý7??'f³É­?0úÎ[Œ?î\'¬ã?"±Æ ³ H?®l 0>d©?"¬²6Y¿uPSR4FGL J0631.8+0645¿ìcù-ö)à¿óêwTË3À8æpÆ;¹À;©´oÞµ-@Ây5v'@XºÍÆÈ?µúaŸF°?â.,Þ°O@"±P¹U÷ƒ?öT÷™Õ¿éâ—½#â?x6ŒGæ7¿ÎÁ ܙs"¿Þœ\W뉿í´bþQÿý¿å֔APSRPSRPSR J0631+0646?kˆœçÄÚA?j_s…l;Â?îéÇjžk?¨Ðéÿ?¬¸Ù½Ût.?§àM¥RÉ÷?†Tÿµ>|?.Rôz­õ?èñtï7¨?¾ÿ~m÷²Ý?Îjê2ýòù?¾¾§5¶?¡ªwʸD?–"…à'"/?êà>ªÆÏ?®ýÑ*ï0¿?Ã!á@*3?¬˜ë'•/?}Ÿ"F6Õ?b
x
ýÜ?쏳M?¡ÇŒOîr?½æpü(?¡|!Ô/$'?tn,-ŠD?pŠÂb­?í1K*ú!?²s,:¤`?µ.Çd×:Ò?±¼@Šµ?wœ=¤*‹'?'›ëÒÐ2º?è©tu»è?ÃÕÏÈÞ3Z?̝L:¯î	?üˆU"I7?–¯*ÿ²J?w(GË/d?ë1ËÄ[††?¬f>ÏþÃ[?Àbë¬$Ð^?ªQë%ŏÖ?Sñ×O‡ÿ ?A¼µ1ãmq?í/-Xíq?¢sÙ(–E?·v¿8Gk»?¢ÔÁnçîPSR4FGL J0633.7+0632¿ä)sÁI¿íµÕڒˆ-À7\Wï«À:¾çW'Ž
@W7•BœÞ@Oú Âî'?–{Ûî}̊?Øp;7äs@:@¿ã°>?þ;Ÿ]¨Ò?侏½wÅ3¿ÀfÌ}F§¯¿Üv" ‹Â¿å½ýûC¿íï@?5J¿ïÿäA2¥DPSRPSR3FGL J0633.7+0632PSR J0633+0632?ŠAçè?4`ۚ÷A?ï»ÐXG"¿?|ÑPK9=?€âÕÞH?{ݙµˆŒ{?z—Øœ_VÞ?ïý‡yO?ì¡QWq½?±öªÜÄý?¹K÷¸ÿR–?±¤`œŠÖ+?rßGâæiT?{ûCꓰ?îZ^,š?šûTDî&?§þ4C–'/?™Z]´×¹>Ê ž;Þ?>Éñ£ãdRŸ?ïr~7ŠÓ?jä2?'»{2ÿ›Q?i
66E?2\¾FYJ?(üŽÛùY)?ï‹E±,?‡l"2>š?Œ›­¹ïÌí?‡,´G\ð?lþhGû?z­~‹EÍÐ?ísSòùå½?²YK™0a?³}m$Vݙ?² mœ†K?m¥®*\¦?f…†@d1Í?îJLN""Ç?œ†Ž"O ö?©€à1¥áÉ?œ6ãúf> Xì3Ù2>§pCËë?ïQƒ*le.?‡¡#ts7?•ÏzÚ³ž?‡¡žmDÐPSR4FGL J0633.9+1746?íüý…b'+@‰I`œÀ3G9"†À9)`ì©áæ@ÄTÉ@gëC°Xù?hC˜ÚLª7?×&v î@l8²êò@µMÏÁžÆ?Àaäáìn©¿Ã2äá¿ÚD+]ÑÂU¿äØÍ÷o7Æ¿î>FVüf¿ïe<ã.PSRPSR3FGL J0633.9+1746PSR J0633+1746?H{€¢	à?H{Iê¦?êéÔ:\û·?Àrg.@é?Ä@3"àæ?Àl{«ir,?''#ßdF?´j¾[ÐU?îŸ04%K"?½nÈ-sù?šòéWw):?³ƒrà¤n?'€FS¤×`?'FòcÒeÓ?ëFŽX.%"?­¯…Åûm?À•½Õ@ÂF?«žì¤4{}8b›!	ºk8¢ÃÐÍRá?ïÿÿþc®â>a¢…¬³>->¤‰ök>a¢…¬³?VÕY;Å"ë?QߍaW?ê
ŸS n©?Á¤Óÿœÿ?ǧ×þaÍÙ?Á›x8mQ4?€ZÈï	È?¦Ñ<•~ú?ïf7u?º§õ<''A?–nÉG˜V?µÓ¿ôxí?Wyš'ì?Žò¥ÓÕ#?ëëIÀpüu?«S"Øœ?½
²½y?©¨{ô=
?8UY›8Lò¨§Jz?ïÿ¯äj"?D_M›Ÿ–?KC¹?D_M›Ÿ–PSR4FGL J0646.4-5455?ë3Nô¸À6˜>·Ë³ÈÀ:º™I—#À<å³Ët9@áÞ¸1µ/?ý¤Uêî ?ÇïÂǺê?íuÉ næ@›ò9?ýJk±ò?ïøö‹â÷±?É|)WIh¿€|Àò+µ¿å…ؼÅÍ¿ïü¶ŸcÝö¿ïÞ?állPSRpsr3FGL J0646.4-5452PSR J0646-54?ÎÄ$û••²?Äå{˜cå?ã"¹F™R³?Ê^Ùýë[a?Ä°õê'?ÀngãOVf?µ `ëϲµ?µFW—tl?êÒÙ
•&»?¼ÕIL?´HÖ¾=<÷?°Åˆ–Ú%?Ë[>7Å?°ã¢bê%»?å|IÛü?µ-''¥–?À®³šPK?¨Ñ¹Þ˜>?ªèË1}?¡ºe#ÊO?é-«Üñ'?§"€m29?±<×»ðÿ?•øÉ¿ˆ3?Ȍ¤Q=ÿ?Á'·­|?ä0
̜PX?È1[Ú=Æ?Ƴ$|ƒ€ ?À³L•*8?¯ªÀ#ð?Ü?µÉ
[4†?ëTV÷ç
?À`
ƒf§?´/ý6H§¿?³GÏ\h•?¾Þ;±K?ªö‡¨£?èNPpŽf?´×_' ä?¾¯`?Û¸"?©ZæqÕ?§¹¯§Û£?'övAåMƒ?ìšè¤Ï?¦ŠèPáÅ?³>šå1
7? ß¾ß&ÖPSR4FGL J0652.9+4707?íIñNº@3¡/À:íu¶e';À=ÊC…Î@¾~ÜÿÊÑ@¥ð¿ñ7?ÒI·¤F›Æ?ïÿ³ß•ý-@[Ha˜¡L@,a$Wοã?ǖ,'?·†M¡sÙ¿ÑÄÌběP¿íðqJ¿æ´|¿Y=?–·Íûå­ÞPSRPSRPSR J0653+4706?éx{‰/¶s?ÂÈ©Û¨?¼3þÆUK?À{£ºY؎?­‡wrÇ*ž?ª(þå™dz?ר\Κû?оl…AüW?á{‡/ñ?ЮJ?µ†[¦ÔF'?«9¤JÿV?âVòéÓ)?¶Dˆ¥hu?Óœ&3?³á·Ù_R,?½ŠV^öo?¦YĜ›e?âƯ–A\?²Ð'8EBŠ?ØŽD¯e?²€÷É©ˆ?£>˜Áò?'ÇÓ
ºšô?å@lx'ý?Ê[kwí?ÐêêhS¸?ÉäŸD†ö1?²PñùÆĺ?­BCÛԒ?Ãöò®;oË?ÈìÉÜc"?è
:¦—Ê?Ì2_po(?·ÀEtN<–?³š?w][Z?Ü·@t w?·Å<yˆ?ÚÉXc™W?¸Ã×C%ø?ÀþÎOŒbØ?«IDkºš7?͏ûqa'?´²ƒOüÈ?æN=_Üßj?¹hzb:Àm?³fõ	ÈNå?§®BèÅÂ;MIXED4FGL J0659.7+1416?ïÿކwl¸@ ‰3ÁÎl	À8U×øyùÁÀ;¹SšÍv@ÝœRÜq@§-ä>ÙZ?§¾Ûrýœ?ߏã=Qš@)vB||R@}¿|ØÚ¿±A)¶2¿ä°Iÿ}y(¿ì~ð€±a¿ï4mÙw¿îøÛH'¿ï§­Ãó	wPSRPSR3FGL J0659.5+1414PSR J0659+1414?¼G€ó™î?Âɍr/?楓¡Ì²º?ЄÜL‹b¹?ÇEðý%&¢?Ç°(ôS?¡`|—€9Ì?¹h/31KK?ìz>cׯ™?¿»"øŸÛÊ?³}Η:4R?¶GÚ Št?ÓÈÿúe?²@ÀlÓN?à±Ûb‡?´D/–D?ÈU"[ʁ?°"ÏdQ?‡HN3¥Û?sŒïÏG±´?îÃØ`Ã~?‰»×/qõ ?›àÌÏuq?"Yéý‹'?ºZ¼Ë3*á?À¦3"ñ­ò?åówÈ7?Ñþ'ÉÀË?Ë#»F²?Ɇ=&&/j? Jè	'ìº?¹ªY¸á'?ìg' 1µ?ðK—ƒñ?´õéüˆ|?½§)KJ?ÔlÅbl©?²¥gŽ(f?Ý;¡kÊÿ?³È~í¦?Ìÿýö)VT?±Ì@¢ô`?_ñŒÁúÎ?SÆÝX
?ï3ðÍ)‹a?‰Ò´'N?—'Õú÷A:?ˆqŒ¸ ÿPSR4FGL J0729.3-1445¿à«ò™‡rr?÷x¡Åg~À9Ä÷øËÀ;|rïá¤Ë@§>9Ìu@÷µ¼g?Ä1§—ß]?Á°å^"
?ùÖ‡å</@c‡8îß¿ï,ýäò³?ì-Óbh*¿ê°ü¢'‡®¿ã\áb0!¿è´y"P\9¿Ü~ÒÃܹ)PSRPSR3FGL J0729.7-1448PSR J0729-1448?çÒÜÑ}?ÅXnæ">?{ËAÀg1?wš!P6?Ðu.Ô…‰?Äþ'¿H?é*H.~(á?ÇΙôé¥?{!ÿþ;†?ˆk'êulM?Ê}ÏEš``?Ç
a"ÿã?êig8Yžé?©›Ép]u?Œp5/'Y?"Œ°ö²?ē_ÌKü?¨§tJ@?ì@ÍøÆд?Ž¥îÝÓ?'0Ùhpê"?o13'lz?¹mY݇~;?‹ÏˆÃýS$?ßgœZ±°?ȱ+þX?ÊÑ1üËo?†Wo´‹þ?ߚöÞn5?ÇÉÞt¹w?äHØÃJ\?ÈÿÁ-~µµ?"ÿ´«˜Ê'?³47y›?ÖÆR1¤ô?Ȃ"H»Ÿm?ẙ¯q¥½?¸½ýÌhÊ?œ¢¨¼RI?ÇáÔ¼rq?ÚÀ¢šõB?·ªC­KI¢?æ¶Õt?£àö45û?¨DÞAÄd?ŠÛǟ7ÿ?ÏrFl?¢íí!ä¨ÍMIXED4FGL J0734.7-1559?íM:‹Ê¬•@')óÀ7Ít9ÀÀ;:¯ åS@³ËÉít@pM•ö?¢ž©_¨ß?ÑÒD2^ø@,ëXK±?ø¨©—h'忳ú§ü^¿Ú+ÎÛ쐿ã·'hÐy¿çpGüó¿í+/#:G¿ïÿå"m/®PSRPSR3FGL J0734.7-1558PSR J0734-1559?yõ°Bhà]?x0òL?ë~ŠØò±?·+ÇãŽB?Á6'ó–æ?¶¡‡»Õìw?'øô è8?¨¹}L¢i?ê'Æfü?¹)t¡ _?Å!ÇèƒÙá?·1È"Ç?²¶Yˆéeb?£ÄVÒŸ?éÉG&…$í?°?@·Ê?¾ÿmD7M°?§éJ€¤?fÁbóÚ?V8a wçë?íJ–²ØZ?šnH?ÜOQ?´õDêY"`?š]›,0?ræêN£?huÙehB?ë'ÍF3.ð?µ‡õ\ï?ÁcÎw'ÿŠ?´£N«ãñ?ŠúÉ¿%?±›2r"\?êçšmvrp?Á»l	4ÿ^?±魿Q ?¿¸9~1?›Aw˜ç
?•IÔ§?ë×jm®?ª¯öÜ£?ºth÷T#²?¦`ØÇå?IR8z¦}?=G7πШ?íoâCµ? —*s?·9Ü~µV}? ƒlۛRÉPSR4FGL J0741.0+6618?ànªáÔÇ@=ŸØ{V¸sÀ:{ÑEØÀ<›'BCJ@͜ùöPª@
U£ ƒ™?½Q°vÕÊ?ÕR%'@Ôà—"ì@3bt>kK¿çT¶:º¿Þ*ƒaHð4¿Û‹ç)oe¿ä'£+Ó¿ì–ÿ'èÒ¿ðPSRPSR3FGL J0740.8+6621PSR J0740+6620?àȺIù"w?à ùáò"?Ú­¿½Q?̍{XÖ?®]uÓ¡?¡‰ ¬ïs?튞¿7'?°ð½9ÁH³?£9' µ–?¨ˆ'+"Œ?¤&£ü<?œICQ¼À?ßPÀ%è?¶ZþaƒùU?Øÿ¿‹Ï49?¶H¡œÝ9?¾À¢ÔÎw?£|Nã›xõ?íöÒôró?‰éð–wó?¨Ék™V'Õ?" Ψá?¥‡'5ªÛ?åðòc?ØØӘe^v?Á§NN9?ඖ:G,B?Ãp]«VÛY?¶çÿÏ2̔?¬]6nT†?è²â3‡u?Ç&DH•?À†Çãa—?ÃCS]#?º7áî-?³s­J÷+7?Ðð×	!øß?µ­@T–Ë­?ㆆ0J?¹Ä9sqÅH?ÁÄ7Ôúæ?¨_&Ÿ¸?èÁˆ€Âˆ%?¦B™¾¾¨X?¾ÏfkU?Ÿõ¢WN¯?»ß쓀i·?šÏ™ØD)oMIXED4FGL J0742.8-2822?Ó-­€^è¡À‰p"XðÀ8êÃ×ZÅHÀ;¶–F(~@&(Ûì@è&ªŽ´c?±vÊâ'Û	?Ôýåÿ"àU@Ôñ€
|[?ýd"äÖ¯?êV?rÖÚ¿²khó¥T¿âTB)Æ"¿ç¡Y{•£¿íOx¾'²!¿ã#͚R&>PSRPSR3FGL J0742.7-2824PSR J0742-2822? Ñ¹P9?›*d'i·?èyVqëo?Âsû|…,?ËM¬R¦7"?ÁdK›¬:Ó? +™CAÎ?¥ûgå£zœ?傕íRÅ?¿€áÁvž?Òõa~o?¼É½'‹ø
?·-¶~@s?¢Ãó¹Ë`?ç‡Ea}?±Ù¢X'»?ÆL`1TG?«Ð—4I»?²¢;ÖO?t?‹øwHè¥?é+yQ5ãÎ? $©Î27?Âüζö'?O+ìá?'Ãœ'ìX
?•‡].$?è_Åé??Àí'ò/ª4?ÌKWGSj?ÀSÑä9?ª€)'›«?'F":˜??åï¢%óôH?Äî'ÍÖÓ?Ó3g²'T?ċä'"?£‰äãÍwö?•rꁉDœ?ê@w»'+«?°´‡cd'÷?§ÙÖÔ?­vHŒX5?'CŸ—(ˆÝ?rØÐ/ä?ëFG
•Y?¡Hx
›Ñ?À¾p‰†Á? À–œGPSR4FGL J0751.2+1808¿¶ÁAþº÷@5‰Å!ÞÀ9]oˆN»À<mByø¢@éR&ht‰@;ÔÂe?³²- ]iN?ç@Íàžö@+€Ïž8e@‡ùw¥¨ñ?ïÿ½OG"?驜œ€¿Äüì$Uõ«¿áà«aG¿îÉ=+¹É¿ïÿÈ¢› ÛPSRPSR3FGL J0751.2+1806PSR J0751+1807?xziù£^?ƒUÊ5§V?î÷!BZÝ?·/Ìٜoá?šýB¶]õ?¶ê÷éDÍp?'ŒÞ±¹év?‹û;Ýí)»?îh.âö›?¦xXƒ=?¤ÙÚ)K{?¤ƍÅ/\?žfoâ˜d?•Uà€?ë"V—}?«K•£Âq½?¿ÅQ‡ â}?©¯î7°?[¿¦ÌB›T?IéƒÞ¯?t~ÆÉ?{C»Æ\½?‡Øíõïä]?{î®`³?‰¢½RÝþ?e­Uy‰M?ï5Í+cÓ[?¡ûàÅ(óÒ?‰‰_iw1?›£êµ¨ßV?'gÑ*–ŠÓ?fïëcO€?'Dpü?§ÝO¹o±?¢'/?£ï†<þç?•9±"œ‹?'‰/õÃW?ëïÿÁ¹Ö?ªÚäX'àú?»1•ŽÈf?©H>0‡õ<?-šª|ó€? ýfß\€?ï±­ðàö?wŽ÷îÓK±?ƒGiØ­?w''04¡UPSR4FGL J0835.3-4510?î*ÑØØÒGÀMCš‰ƒ¢À2{Èxª5ÉÀ8AA [À@ä¥}'ÿ@_ø"»ì«?gÖƒX/Y?Ô@Àæ"t@j¦[[Õ?øG>¾×?Ÿ
fÞõ¿Ñ``'çα¿àQúž—/\¿å£~IÜî¿ìö
Ù–ó¿îϼ5¥Ô:PSRPSR3FGL J0835.3-4510PSR J0835-4510?"ôÚ·þÌ?1F'4BKX?îX>ʸlæ?¶63Ù m3?ªiu¸ž*?¶,Ú­ÏËI?€‹n]«¬Â?¤Á¿Œú"?îîcr7¢P?·Î>=²¥ö?™íڅê\¢?´®÷¡»Ü?|êNîõž'?ƒÙ¨ï<Ð?ì·×L$P?¦Ö^[€p?¸r ®Ò4?¥êGxbÝÞ8e1A«æê8¥+ƒÒà"@?ïÿÿüÇ]Ä>p…'ægL>;"$'`>p…'ægL?>e¾y%è?Hн/¶ 5?î/$$Cù?´q«=˜ØM?¬Ë"CDúæ?´aF1ù³q?qħ'%?'揠ÚF+?ï8ΤN–?·©{0µ2?"u¬ù¸?¶¨î=ü3?m«d¼%`?sNݕX?íCÉFÁ–Ÿ?¥LÉ÷Ï<»?´ôZ¢ÿB?¥Ž‰g"±8ÒüÝW8^MtŒÔ0/?ïÿù"ÒN'?8Z>Oʺ>ËuÀoö§
?8Z>OʺPSR4FGL J0843.3+6712¿ï¦'ÍǕù@AÍÀÀ:hf9ñÀ<žSËY/F@Q¨¿&?û{Ɋ"-Q?¿-ý¿3?Þë¢ÐÏç@ªÉlÅü@Æfªƒø¿ç~è¾Dô§¿ÀB)Æ"¿ÆšXz"D¿×B¹ãæﹿé*æ}Íá¿ïðJ¶·ªPSRpsr3FGL J0843.4+6713PSR J0843+67?ÒÀ
×YÉ?ŀ…M©£t?æô"î½k?ÆøI
4?"r?‹G{˜*B?Ù·Ùö€û=?Íé[x̚x?ßø`/Pá«?Ís2-4ýŸ?¹?gÜ¥`?ª›f½3?ÚP"?Q=y?²~‹‰&(
?à*y§Gt?²Ä¥0݊¹?µiåËòt?¡˜u2É?ãÓÒ·¿ÁÄ?ª¼Ž0ä—?Íuùƒ†-?§&™Ïwá‰?Ã:»zyÄ?šžé™ôù¶?Ì
|$º—?ÁUwÖ¦??è5H±Ê'á?µëΉ?˜ë	¶¨—:?M2¥Ôk?ɲ[É÷§¹?Æÿ`=,†F?å£æwvaº?Ì.ÂÖSß%?¿|°]¢À?¶E?Ü+=?בXv®2?³ŽdIe*¥?ᳫÈpG?´æû¬"!?´!Ú/Þ?£3'T‹#ˆ?Ö=ÛJòu1?°€U]§€?Øø8?´øL\˜ë?Ѷ¼Õw°?¨Y¦í¯šMIXED4FGL J0908.7-4911?ïâãóϤ¿ï™–òö,À8‡oó­â&À:{ýÍpa@XŒ­@C\ƪsÜ?»Ì뀗.?à—-¾ªN@!iÓpô@ ôÆ/$?ïo5ýè΋¿ã6oÞ_Fb¿å–Ÿþ7©¿ìtáMK¿ëî‰J–ý¿ïþ}ÿŠ9TPSRPSR3FGL J0908.4-4916PSR J0908-4913?•;!Ûoq?£üÍÍQ"?í€?æþYë?·æÛԘc?­^q˜ô˜?³>ÆF°D?¯öÑψAl?ºj3$š"?àñî´ }†?Æþζ¼%?ÚH\²ç?Ŗ	ך0B?¸'ÓÕéÞ?¦>ä€w
?âP^ƒÝ´?¶5l݃?Õ;}^G?´pùsf-?ˆIg畱ö?kõá,yw?ßýüo§­®?ª|*Z®?ß?¸P­±B?ªG™|ÖNÞ?‹¤Ã`•Ö'?âã!"q¹?í'´o2è¶?·IjòC'=?³MÄ
Í?µÍERÐ?'Pv¨é?œ…5Åߞ?ãYm=´Û-?Éñ:Ñs`Ü?Ø8p"h?ÉtÈieÊ4?±T*OŽýl?¢óÓÂwn?ãñêCˆÉp?¹Å"r9?ÓÇ åA§"?¶î:fËiŠ?\Y¡Ð€{²?F2P=€:¨?âú>¤D\??³'V¬7•"?Ùï)|µ?³‰Ûm»PSR4FGL J0931.2-1906?îŐ &Ę@78ÿûÎBÀ;Ñ‹èÀ=nda©h@@¸MŽÔ@ºÃ.¾Y?ΦKÄ#°ß?ïûK€1È@æ…ý¢ý?ø^ Ò]…l¿ì"Ì3?ïïWq\?¶Q'ľ5…¿çVü\'¿íü'Ÿ½J¿ïæ#뗓/PSRPSR3FGL J0930.9-1904PSR J0931-1902?º&Jíd	?¾Ø#­aÖ?êÄ
j: )?ś]«¤*?¯r"Õ÷d?²H|Xô–s?¢N²ûÌ[ç?ªkíÀð?ílÏ
f<l?±ÕŽ'%?¦ä\)"ZY?£}gš$ I?Éôü
N"…?±o‰BŒ×?åÄOY71?´c/M?½õ
j™j?¥ç\ö/#?®š­ÌÉ 1?'¢åöþõ?ínÿ*q¡?–¡Ä_Ç?"êÁf½y?…Zaèœ.?³?'«S'?·ÉåÀþQC?ëi•,Cø?ÀmäkÇÇ?±sĆ¢Þ÷?°«²wV?•ØM¤ò"è?©`+i\?î\ºÚË­?°ïÕÃôê?¤Þ
{ŽwÅ?¡WMRoî¸?»öBÚù"Þ?¨ýœ4"âD?é*$!®Œ¬?³¿jG¶;Ö?º¸œ'Â?§=@7´›?Œ/2–¬ß"?z¤28ß2?îñ{2Ùϝ?Œ¢§zÑÚ?"¹\ß8'?‡,q/ꔹPSR4FGL J0941.1-5429?ރr®M¿ô‹'!¬ùÀ8úH…ªÏLÀ;µÛSñ@Þ)–|Y@Kh¢×0?»–ûÁÖz?âüÖö@"§â?$Øý@«<UEצ¿ïí×Äw"?ïÝ̙¡&V¿×?›ÜÀ¿æ{:ˆ&*¿îgý?[_¢¿ïÿýFKêPSRPSRPSR J0940-5428?·âÞEÀà?–8ÀsŸ I?îìyá(¶?¡†|ví?'ÅíÞµðw?¶àÓ0!?¬eZÖBö?¹3]øÊ$Ó?äÒ/ŽI? ?ÈÇñ4¤ç?ÒÙ8œ(À?ÃÔµ—"Ÿ?¹+^ìÌ%ñ?¥p€¿¯¸'?郡ìé¿?®Ùð·7º,?º·'«}`˜?¤WµÚ©?¯è³­æ?ãiJ7?êÊYåpÿê?¡Í
¾žO¦?¹¸áøôÂ?Ÿ=T³ÜG?‹û.
ߔì?ý oßà?îÛ֐ý?œ+\Ìíc?–‡–ðn}ç?"™-uõs·?‰­»Û·É?"–âBz×?煢‡1•­?ÆI©*lv?Ð'MY	©?Åæ*¹3Š=?±zŠ_QåŸ?¤s¯â÷ªž?êúŒäˆÿ?«ýù2¹ï-?¶±z¶i?£¼HïRÌ?Œñ'T"Å?slÁ˜gõ›?ì¢Ý5áÊq? { só)É?·Jä$¹:!? ¤(­PSR4FGL J0952.1-0607?È¥!Óörõ@A±tÿ†]}À:È5šì€À<ÇÃqÚ7ï@xJ7[·@#3vO¶?ÇqØõÏûU?åÑneZÎ@›"ªNô@¼½{¿í½FG.?ï«᛿Î">ï)¿åû«©g¿ïÿþÐñ?ïÚ?›Ü?PSRPSRPSR J0952-0607?Ó©Y¢€…?ÅeTš®cø?åOs¢'÷Z?Æk›71"??›{ñN p?¨j6&Cé?؟'0#;ø?ÌfËø!Ë?à«U0‡?ËûÕ	B…?¸(ºÛÉïí?¨^ÿÞªÂL?ÖÿìÖ×Ú?µ—"‹áÀ½?áC¯=€û?¸«õ"¾©Ï?»¾/-Ș¾?£ÂO44?ças;ð`?©¤ˆ+¥MÁ?Ëüë<hTí?§Ó®Lð"?©õ!ªŸ¦N?‹"¤'Ū?Çueۄ©%?¿Ä"€;_ä?èøvÚã÷ó?Â&d]þ8?¢¢úåeª<?¢ð]À»?Ç ù8ªZK?ÄJ³`Ô?ærÄK—%?ÇÓ@;PÛ\?¾'ì"N'E?´áçÍ?t›?Æ!ËþNX?³3œ&Ì#ƒ?çS7(òN?º†ÜEÄ8?¹!诗·á?§tz¢ÉÉ+?Û8Dãgv?µún•É²?ݛøÏ403?·»©Ë×3¢?¼¯	5'dõ?¡bûðVJMIXED4FGL J0955.4-6151?â@Y[³QÀø*ùÀ9ª¨ââ¸ÇÀ;ñ롤*@ŠÍ²¥Ú@ ` SÇþ?ºCSyO?ÔÐ=ºË˜o@»­ˆ["@ۄl5Þ3?ïZ° F\¿Ñ,b´€%¿á/âjmÝ¿æ:"ÀÅ¿íÎôÅ9Z•¿Û‹<¿N	"PSRPSR3FGL J0955.6-6148PSR J0955-6150?ÉÆ(É?±¯GúT?S?Ùûö°öØd?À†¹‰	d¿?Ùt&;Ã?¾PEìã?ÑB(a¦–¶?Æ"<wÌâ"?Ñúp)ïÎÁ?Áä9GkÆÅ?ÜÃgtišŠ?Ãå1ùÞd
?Òz6¶åÀ?±ÑöÞ<b'?ÞûOónˆZ?´Äû¥°Üµ?Íò«X³Ë?°3•©?ãNæ3"ñ®? >QßƤ•?ÌSœÀ%Ü?š>é‹#©
?ÆqN—Ôê?•:Îsp.?±ìI¾r¾z?Ÿx/\Q2?ߦ[ÒlQ•?'Vd™:W?Ûޑ½¤ˆ-?ÁyôB‡?¾®Pññ/¿?»'3ô¤,E?×i0h?Çô¹YÿÑ?àu²ÉÊ{?ɳ´‰W?ÀŸŸ!î½8?¨:™€¤?äV›Si?¸'°¬'¶$?Îø#ƒ£õ#?³y–{ÏP­?Óg R›Xa?¡ƒ*rh~ú?Ù_‹îW®_?¦°¹Ü*?Ó8ÓÀÙÿ?¡IVÆlR½MIXED4FGL J1012.1-4235¿ä;OŒZA@&u֝0'À:ˆ­¹OÀ<u¦N³Â:@,mÇ-Ñ@PwFˆz?¸c±€@,@?Ói^¾Q^í@»hH¾µ³@¬OТÅ<¿Öc[ïêß¿áöуòÖ¿ák#>ô\‰¿áSµõòð¿î¹ý‡»¢¿ïþ÷÷óÂPSRPSR3FGL J1012.0-4235PSR J1012-4235?ÝdŐÝ!H?ÃBÇbL?ݶŸ`¥S®?Ãz¥oˆŽ?³'l9ö,(?£õ³ÚdD`?ّMÍ`?Ê®©ØùMV?ړÄ4U{?É×![ç©¿?ǶÊTÕøÎ?¾'€­–?ÜFk•‹~4?µê	ßiìà?Ú§¶¿çƒ?µMXŸê›´?Â#»Uüš?§T»œd¹?è
-ìUô?£q
àóˆ>?IJ‡~[r?«É"ßFy?¶I¡ßÀ?šÿh,C'Â?ѝèr3'î?¼ÆÜGê?ãnÂÓ¤­I?À7ÜL?¾GšIÿ?­(ØüØo?̓)tåÒz?Å]w×tgþ?â ª€5‰?Ë24}«?Êì{Þó•ä?Á'"ð%}¤?ÐÕq›ñ?´UØFç?âœM{]ïI?·˜Êö'F?Ãä¾¥
ø?©·ðõ/žR?۝lÄÆ»]?±A}}ù
?Øvþ©éé?±»ø#0¿b?Ç×)"ŸMt?­šMkQÌMIXED4FGL J1016.3-5857?Í
'ºóË-¿þõ™t°¬À7dÿŽÀøƒÀ:;ƒo‹©@>ôŒÚ@cäõ8?©)·ßTä´?Ô°ß¼ÀL@$ŸÖ¶Zš€@'ð,¯?âã-ÌÁå?ç.ãBZ¤¿á×ûnÕ÷¿ålÚß4-"¿ì3Ô
2îj¿ïÿÞÝpˆÿPSRPSR3FGL J1016.3-5858PSR J1016-5857?_ï®u'?_uÅM~?îDÛ%^?®ÞÓñ•jF?ª¿˜®MŠì?® RZÍ?ˆ´"Ñö°¶?'"Š‹¸1?è)gçè(•?º5Ŭ'$?ÍÏ#vì_?º€·I5‡?ž«Ã¸ˆ…?–4úÁNTÒ?éÖ	-j
O?³ýÖOÅu?ÄÒbÒ¡ç¶?²Ú´€ …?m ¿•d%M?T­g!?çAÛpîC"?¨mq÷­åÆ?ÑAžÒ5?¨DåtNáƒ?\xA²‹X½?V'Ûÿ)GJ?í@…/ž??²*ÙyVα?µ‰õ'Ó£c?²#DÜ0¡?wÏQëéËF?€wF2"QÜ?é0ŸL¶çÞ?ÀÒ2XS?Ê>	m?ÀÂZ˜|ä?‰í6KVðœ?ˆº½G÷úô?ëu'pÛ_b?±•2¤‰þ?ÀŠâ֓8ñ?±……í­?EkÒM@Ñ?5"Ø\½Q'?é<,ö¥…­?¬žW.ë?Êú6¹
ß=?«úG«Ñ"¶PSR4FGL J1019.8-5749?ݽÔü
¿åþ-BƒéÀ8u2_Μ±À:'
´©@ÿ¦|V@¬øCsW?¹Ü<ŒAí?Òhm
&Ú@Ýø?A^o?ú[çW´³?ï…/‡­¿è³ÿ ‡	¿ãíê‰v5ç¿ãØÇ«â¿ì:"å$²g¿ëDõÓVTPSRPSR3FGL J1020.0-5749PSR J1019-5749?³ó&ß°Ð?°뵙u?â:à"BM?ÇZˆÑd%?ÖúÀ†Ô2?ÈróûÃbô?¦'X/1"ú?ªa47æ?Ñîë>Á Ž?À+Œé»xš?åŸd݂Û?¿ˆ"¿?¿YΊ^Šœ?¦ÿÑksê©?Ö.Iì'þ?³	–ÐÓ?àý¡8te®?³:5 "ÃC?–½ü÷Î2q?t—=s#öA?ÖÈ{Ù.ä?ªÁAÅÜ?ãåÒ+JJk?ªÜ™™Oº?¬nù¦ØC?½SþÒ$òË?ât¨H‰?ƦʕÌÔ?ØB	âySË?Æ|¨S4Ÿ?Š³}å@ރ?' #SDµ7?ÓÌJÛv¼?Ń,D×ur?å¯û?ű"9ù?²±Gëd,?žÊ选=±?ÙDË3?¸8rBŠ?áɾý?¸?ê
Q;?q¶üi'&É?YTN`1*\?ܞ‹eB<?´H%ÇZŠ?áLTtÿå?´9·aϪ'MIXED4FGL J1023.0-5745?®ž°ý¿Ùv0¾ŽÆ'À6¦|µ]DÀ97Ó«ä@•#/Úä@W†Üþs8?¢äý› Ø=?ÖÐ6
Ù—@3hî9.÷?ön¼ÆÅKÏ¿Ì,û¡ ¡‹¿Ø …Üxfn¿ÕMý¹Ô¢"¿èq_=Ó¿íÇHɝmd¿æýsþÕ]•PSRPSR3FGL J1023.1-5745PSR J1023-5746?a´å?¬]­?aˆwwvª9?ݞ€±ô·Ö?Î%%Sv ?á
ÁÇW?Î&¨úúK?rØÞrKæ?"4äéB1?ênŸŒ¼€?¶ÑÎ7õ©?ŰƏy¾?¶øeÊ褢?"5ýĺ¥E?'P6ö¢ŽT?åًl㶧?´›‹HÌa=?Ó	‰IGû?´[àØEÇ>â]eÏ{>Úu91ÆAÐ?ëîïȋ†?§l»>TÛl?ÓûæÑìØ?§lq—³?`MHK?TR¢0¹R¿?Ú(W=X?ˎö·Q?âÛ¾êáà°?ː(IÓ¼3?jPÆ5hË{?vÛúÏ­êl?ë‰RÜñ³?¾Ã+R-
C?Áqqtþ"?¾«iú%S?‰»a}cý?ŠÕ¦.5D?æyor¥˜?·D 
½l^?Ò?F¾ø›)?¶ñàÚ*@a>±A9SAf©>±@)CU?뾬¡ð;x?ªyþ@ë¶?ÁDØ¢?ªy{
±MIXED4FGL J1024.5-0719?î.슊æ@D?_JsÀ:&­czù›À<nÌ¢Ûa»@²r'å¢?þ6"çƒ1x?Á …¸Ò?ÛÛO\¿l@Ô»ó¡M@'´ªA2?ì<+)yv¿àš®×ï?¾¿ÖrÆ{ÏÚ¿ãfŽàV¿ð¿ÕÉg}ΊPSRPSR3FGL J1024.6-0718PSR J1024-0719?åV JD¿?Ì»Ò<?Òð	Ù?Í'Vö  ?ªŽzŸ¶ò£?©Cý$ÁEÿ?Ôã	"ãÿï?ÈéÓi…:ù?ârՀá£?É?J½,_ž?¸Ý-èd ?«T°è[B?Ð{vµáEL?²8,¿—(R?ã, ÷5Dõ?³ú.…©– ?ÂXŽ·ha"?¨?f®pýT?å9+«æ‰?¦ò²³Âð?θ"Z"?¥°ÂFŠH±?¹ö0]ëÈ?w!¡DƟ?Þâ&"˜?͈—¶
w?ÜùáÏ#¥]?ÏÃ[+l7?³Èð+C,?²f[ѐj—?ÄH'°sû¥?ÀüÕ͖:-?ç0ý¯©âx?ƐsËSÐã?½ç
!Èôó?¶‹ˆLfÌB?ÁÈñžÆݨ?§R°©
¨?æe¶¬`+ö?´QÌ9·®C?Ä 3¯¸r€?°o)×G'©?ÙÌÄ´zp‰?¯H0…ÙÉ5?٪ݳ=ÉS?²kmb3Dß?É»2µMÄ?¢5X:ÀMIXED4FGL J1028.5-5819¿åö¼¹šR¿ßz0ÓJjÀ6
\ËOÀ9ëQ=à5_@J.%'E•@%Uœê†ò?'Z,œ@=?ÑO>šõ@<g†ø­?ûð¢l¦òH?ë\âŽÕñ9¿×•Ù[%•'¿áåNšDº¿åu'¾´V¿ë«ä<U¿ï$à>ï~þPSRPSR3FGL J1028.4-5819PSR J1028-5819?€–®|-Ž¶?µq
A-³?íWÖ6
±'?»Wµ5Á?³.xçŽT?³*VdÂu§?kž´S3Ϫ?wbD³"ð?í•ï¯¿?²É¾½ì?¶VZá'@Ä?²Ž}ÎæA8?˜™7_Fs?"¡¹E'ô³?é½à"f:?²÷ÏîÿÍ?ÅõVÎî»	?±¬>êtÉ>¦IÊ
³ûã>ªzeŠb?îèV°]LÚ?'ó5ÉO:?¡z~­LW[?'ó×·Lã?oÌ» x²¤?®IÉe£Ã ?î6Ϫ3?²0	ݸþ?ª›7HSœX?¦U»•º3d?`Ï´/tß?pHlϱ6?íã÷*TL?²£Ruҋ?°YÉ
ê=:?²nð"Ï?ƒ¹Âe?ƒŽ‹åÎã?ìIúÓxì?°YøÈ<êù?½$8ï_É¿?¯"[ː‰;>~S¯ì]Ís>‹^ºu?Uï?u™xü?›k­Ó+nj?¦Ç"ÞR"}?›kª'nIƒPSR4FGL J1035.4-6720?̘ü%Tù,À`n¹ªÀ8µØGTRhÀ<µ™ª`'@Œ<‹v–4@ÿ‹eú/Ü?©Àc‡ä»?ázM£÷Á@0o¸dàT?ùL•Xí,?ïöÎ}üÛ?͔àwN–¿ÖZÆ?iøA¿æžvx,¿îjÃê¥ü¿ïÿüoQÇsPSRPSR3FGL J1035.7-6720PSR J1035-6720?btÝÓªiz?pŠSð0îÏ?ÖÐde?³]~†ÿÊ6?¢í´²{r$?²ˆòÈk‹?"C̖B¸g?Ö­_ïàÀ?êÃD`ñÌ?ºÛ¶µwÇ?ï¢$W£*?ºÌð‰'2??Îü̊?­é¹•Ù?íw7ú?¥mÛáðG?µ·¢b"Üd?¤SÓ)ÇÊf?2'ˆdƒ9?#»ýû*?ï«RxÀ'š?q4ê5Ê?"–ÕŸ"Rb?q0æŽR0T?`IƒŒH?hé>ۑ=?î­Õß	L?°ir¹Ÿ¸0?¤Ã>?¯¤Ü÷Dù?z՘¯®Ö?'õWÿr?ë;	>JÇ?Ã)	`¯v?Â=.BÍHâ?ÂôH§8¾?|E [˜>¿?x¾1‰´?í¦Â:O?ž«S~¢àO?±¢u‡Ø?!`}Rñ?󂒗4>ýÅªÜïÍ?ï­Ù¦"ÁØ?s#ﳧ?"qxnæU?s^â\,PSR4FGL J1036.5-8318¿ì JhLÀ5'"»äG=À:Dã)/¤2À<‰æ¤å'7@óú0ÞP?þÿ ÜïYÀ?½ršÀúËR?àЍK­}|@Ž½'¬î
?ãq÷ÝØÊ¿î7ûþé?ïýÖZHŒ¿Àí ÂWÓÑ¿æ6™ºPÉF¿ìDŽ#ρ¿ïÿ®¡hšôPSRPSR3FGL J1036.0-8317PSR J1036-8317?ȚÜý=û0?ͤXBÿD?é?ë3PuŸ?Íõג?"+±£jlŸ?¢1+~ï?°ˆÓ?µ³ôÔ´¿é?ë â8ÍY˜?ºÇ|Œ4º?²ief!¢0?ª%= ?ÁÎðØ3¢?ª¹ýû˜'?灂Ëá?²MÕØC‹a?À+«.t?¨÷µÆM?¬"u|ԝï?Žçìµ`Ð?êXê`»p?¤µn£õ?¾îôûü ‰?¡fú§Nٚ?¹fã:>ß?ÇGözÉR?ìjo˜qÙë?ÇhµÄz?Š-D"p?‹JYÿ¬œ?¥YJ"ßáÌ?¯)‹yý9U?ìE£5ñ÷?¹Ž³—F®?³&mªYâ?±%ýÃT'?°®W¬—×? wÛ.¿z?êQ{F-?­ƒS:\]?¼Å¦yA"?¨ªWÃ?"Eè¿"?ö'-
]?ëMD©¿*?«s»Âñÿ"?Àb0E[î'?©X: .ÁPSR4FGL J1044.4-5737¿èÇztT)'?ò€]£IEÄÀ6õ€ø¸ãâÀ:jýKð™[@Ôä'±@ΕY˜øŠ?œËux–Ùe?Ôb«Ü<Vr@4B†ƒ<`@J€y·üÜ¿¼3@®ñÅ¿Ûv·¢CC¿ã9Â~•1U¿ç
ŸÎ¿îYD_*‡é¿ïû•"d~PSRPSR3FGL J1044.5-5737PSR J1044-5737?^f1‡ioË?kÄÌ)7& ?ë—îªÔ?Á]ZT›sö?Ác{Uòáñ?Á!p—[•—?wdE™Ñª?†-œÆ?é³b¥^V?¾
ËÁE@b?ÈwS;ÄÚÄ?¾Œ¾ûäù?–²°žÚ)?"qw³ãX?됩éÚ
?ªªrg£Ä?½Ó6¦ã·©?¨•'lâS?$±˜"¼í?­ÇÜGž
?쀇&8?¡-TuBå?»ñnq¨3?¡RÜ«D?ZǞä€ù]?V˜RËj©B?ëþ«Ï|)œ?½÷Éòõ!ø?¿Ÿƒ
"·?½ÂÄ`A´*?pvlË\æ?{éQNd""?éÍ[-0?ÂÎð0²­ð?ÈFO-mã?ÂÜ'-B?†šË¾qú ?‡BÆ°gõ?ìÅ÷ÈgÒ?¦äeîçìÈ?·Éî'?¥ÆžÂDÕê>ùD[X±¨>ú€x"bK?ì{þڙ?¤ %Ôï¾¼?¼&.†ìw?¤ŸZ෕wPSR4FGL J1048.2-5832¿š=p"êŽh?â^$ãåFÀ6_c-תÀ:?aÀxi@ýÊE³é@Ñ$šéû²?'[r¹ÓBT?Ò¦‰l$ìI@<"™(Z'@"›NÐrŸ?ï:$n:¿ÍõX‡*¬&¿â5¹ö0s¿åh2^L¥¿ìºr•;f¿î¥¿—°
PSRPSR3FGL J1048.2-5832PSR J1048-5832?<—ÝyÙ?@ àâÌV­?î§R/ÞÑ?¡½è»7E‰?¥Q®â?Ë~?¡™˜¡YÓò?tܾaAñ?Œ‡ïøöÌP?ìÝ3'R\ø?µ-/Á—B/?·ÈšÝ€=?´ánÒü—?…Q}@à?‡–ÇԫÇ?픦»É¢Ô?¢š*Õiôþ?°¶ßò
ÍM?¡fÚTŸ¿x>¶Ûâs>ºÏÒ¯ƒ…?ïTŽ@ä»p?"OnSû?•mÜlöúþ?"œÂj‰×?<ÓÀ7Ä?3w?Û¡©v?î¿ÞË/œX?ÛÖ4g=?£ÈkÐCàç?¾{xÃu?f¦Â}ï¾?w44€‰T?í¿m•Ò??³Oó7Žš?±O]Akފ?²ØV|e5¢?vORnþã?v'ÓoX?î(qÞ¨?('ý?œ¨?ª¯Á´‡?›À5%*ûº>‹£½¡wÛ>™h~‰¼ÝŽ?ï ¿ð©K?'±§Uº‰¹?›è‹m¥Ù?'± ­|RöPSR4FGL J1048.6+2340?ì5E½W›@O0¾
í)À:5¸H±JÀ<X•âTô@®°¬Õá@5^³¾?·ïðh]a…?É^KòK@
yT!ÀD(@ª¢€s?ãÛÀÛ|é¿ß‡¢u‹G¿ãwr'dÈ׿âðc	º"å¿ïÿBu?ïƯ²	ÒèPSRPSR3FGL J1048.6+2338PSR J1048+2339?íE9½æÕâ?«xHë5õ?¬—8>«y?¥'w}Ž@ã?Ÿ3™Ò§ì¾?"¼Äç²¢?ìÙ￸^£?¼sñ›?ªk}<?´¤ÛýMeg?§õ†ˆÓuI?¥§ª€&?ëHƒÐ7C?ª»Ëi?·Át€º¸?¦\¯á+?­r@ŠY1?—̳ç‹]?íÇnú'5€?Uºn;Ìÿ?¤¦Ðb#MÇ?ˆ Ÿ4_?Äë*'v?|	"^W!ó?è"4hΆÇ?¿Ñ»½
š¦?Ä5
2Ãv¸?ºZ¥
Ò6Õ?²ôBTàÃT?ªßÅ|:Qú?èõïB:©?ÇoÔ:÷š"?»
Îû{6?ÁOÙi	Ñ2?½E¶îi)º?¶«Ó"f?æÆí‡#î?´ß;ã
´|?ɃýTmÚ=?³eƒ
J¬ƒ?¼)Íêë,?£f$ÿÂ,0?éâä€ÀÁ?¨ó8ù?»½àBAæL?£ìRÃÚ%t?µ*þñJ .?˜Þá9zÑ×AGN4FGL J1055.7-6028?ïʖYѶ¿çŽ2BrkWÀ8¬À¾¡'À;˜À¤ @SÃvŒÏ@*]Œú?·³%ë!!?ÔÀÎý(µ+@x_»Qz@êǧŽ?èþ2Ö!ª¿ãÒò䏿ÕØǁß=¾¿åÁßԍí¿ì•ªåò8¿äaSlŽž"PSRPSR3FGL J1055.8-6025PSR J1055-6028?žzÖµ?"£Ð$&B?쵌°ÁÃ?³qõ*'U?²µƒÖ²Ö?®cªRÝ7?«ý°Û¯³?­YÒ¶?ۆ¶'涝?à7´]{l?à‹´Ûƒ7Ç?Ã崋s¢?¸ühüÛ»?¥pl~ÍHD?æV`èUÇæ?²ëÆ}vz?Ê(Gá"Ùˆ?®—ÛÀx?³v)óð?Ãµ¶€''?àX£qƒ?±%ª2Pܨ?Úq.aÎb_?±O"ÉUgô?Š™æ9öÀ?ýˆîü?íçáüú{?¥ý¬t¯Ù?ªÛœF½Á§?£3¹Ö?YNÝ?'ø¼…Ó?Þ›xtŽ{?ÉS•Ïñ«?à€…áMYÇ?É@'žwÇ.?¡Þ2gs?•Ú3 hJ?éE‹ûKe?³)Í"'P?Ç'dÂf0O?±o«ä%Ø"?SJ®8²Û?s<.à5Zæ?ãw'-~?·WŽÞ¸?Ø;‡\M?¶ÕƒïBMIXED4FGL J1056.9-5852?ís–r<?èîš|îhÀ9×AšÕÀ;Å<¤ËüÃ@?bØè9@ìåÜhKC?Áü	ÂÌn?ïÿæÀ
@"vsBí»?ö–£Þ S¿ïú˜i²?ïþW‰SÑ8¿Ò
è@EÀT¿ì2j€§ZL¿ïÿû-2h2¿ïÿ'¢."'PSRPSR3FGL J1056.7-5853PSR J1057-5851?]ôÁv@Ú?iRtq"?ï*[
ËMN?§
ˆâ?ºP?˜ÕR3Qܯ?¦M¶ žB6?"Œg ÛÔ¾?«6d$k?鳏á"Þì?À²¶ 8Ò?Æ 3†ë9?¿GWúµ4Í?¸ÒK÷+?¥x±Z•¾?æÞ{݊Îê?±â}KÐ–?È~ å?¯"0Î#ðè?S# J1¤?>6œ7ÆMQ?ïmÔjŒ!?{ó*àûl@?'8­JÅY?{M×U'/Ï?m‰žÚ`0?{ø.'Öþ?îˆý'LK?´‰CCÎ@R?¥—OD9T…?³¥"ßܤ$?~x¸jk‹ñ?£ÏªäÏàÄ?ë]ΰs?À´@wGë?Á—»7&w?À+í³f
?­…·WN?Ÿ?:Œ?è"¿|πÔ?°²±´ì¦õ?È/`žXùŸ?®Eùóò6±?&¤'Ìø?'6òUà?ï £ï2þ/?|%ö™b/?‡|qßye?{ëø…é¹PSR4FGL J1057.9-5227¿ïÕwxed@•ÜÆ?À5òtBÇüÀ:ÄëQóÛ@¿àqoXþ?ÿé}£~?†NY²×`Ø?áRqQ{ó–@TM)Ür\>@'Îunl?˪OŸO'
¿¸/g¡¤Õã¿Üà"È×˿钂¹ƒCí¿ï¤ƒ!Ýö@¿ïÿª9ú͑PSRPSR3FGL J1057.9-5227PSR J1057-5226?2ᖪ¦
	?B½[«ýhY?ïÅ]²±Y?Î™m´?a?|#
S)7§?@.nRn?lf~69X?¦û">§?îºEö·à?´««|²J?¢˜£Àá?³¼Oè½Ç‹?™}´ª¤ÖO?–‰SB £?ì`ø?©›.ò–;ê?¹G·Óm/@?¥Ìrq}<à±@Ù¡f=ñœ??ïÿÛã8¡?oŸ•K>òq~58˜?oŸ•K?@¿ÇðÙ
…?@	Îó¼?ï"#@Kõw?ÁoÓJàç?Š+3yBûÂ?yi5*?t¾ðVAé?–{—¯ð¯?îÕJodç¶?¹`KîΦØ? )á*éb?¸zØä 7Ÿ?‡"¬"¡|?ˆ‡R²8þ¢?ío9ÁJ?¢;&vÖ-ñ?±¢M¡GÀ? ö®ªH<«ƒµWé>Œ<ØÙ߅†®?ïþûà­÷—?>#Ó~ÃÓÃ? A÷tÀÅ?>#Ó~ÃÓÃPSR4FGL J1102.4+0246?ïü"$(˜@K+J#9ÀìÀ;NVCÙs¤À=Y/F>©@b«@a¼þl'?Ô¬Ù<qËI?ïÿüÉï£@5‡†qž©@'H¿·e‡¿ìäšHì¿ÚØÐ;AI¡¿ÌoDö³¿ìoç¨m¿ïÿþˆ0»Š¿äðŽ¾^:PSRpsrPSR J1102+02?êu°äÂj?ÉÜ©!)£ñ?Àz¨PY?Å
qF·?­¾´ª?½*K(Ùy??á3í¦>Ì!?͂W£lñ?Öá=,[R·?Ìd\9ÖB?ºÛžœT?±OPP¶?ç%Í;~ÿ?°õõùwî?ÃÝ㕼n?«D_YÝ?¿ã
j«ß0?¥ŠAv'ºu?åšÒ7߄#?³^'Æ5s?Ò[g†ï?`?±ìPlë@?£w NÙEÆ?•Ư`Ý?è1Ñsûz?˖@¤\?Äèx×?Åøß`‰hÛ?´£L"i»î?À.NifîC?Ô2žÅŸÔ>?Í?‰«˜}B?áJµø?Ðyü'"fÌ?ÃA—¢Ò$?¹ˆZðcS?â鿨2Iå?·,W¶p ?Î$mló|?µAûq"±—?Æ4çñÉäï?¨wÖjEª?Ô¢BÂi¾Ø?¹"­!ËQ¯?âá/k:/?½ÂH"C?¶myŸy
¥?«Í5[å*¨MIXED4FGL J1104.9-6037?Ö³5¶_ö¿ÚQ¡GãÄ`À8HzÿzŸÀ:Æ:¸b²@áTzU±@õ´'S+÷?²×f®µµ"?ܼñBM@"ëQX¸'ú?øß',꙼?êÃ'ëk¿Ó?¦n£¿ßÌ! Œœ¿å‹¡¿ï¿íBÞô¾¿ïÿÿ)@k*PSRPSR3FGL J1104.9-6036PSR J1105-6037?J‹mŠ8"´?Uì'OüT=?拾²ۘ?'õ·yóô?"ê\±…h?'<
ÇØ?Æl[=?ˆí{$*Û
?çâ'U[å?¹mÚ,&'Ÿ?ÏYSêt
Õ?¹e÷*ÄO?'RŸ<ÏFØ?I–Θg?ìxùë¶>b?¨€ܚ
³?·£ˆÒ>T8?¦ÓfP?eƀ!äY?JÖ;Øz9ò?èÛXì³Ð…?£ûñº(.?Ì>2ÇÂ;?£ïß	¨ÿ?V%aãC·ˆ?LËëm"œ
?ïu¯Q'Ã?ˆÊ&¾Öv?Ï[_44?‡'¾oM&
?tâ/@Ol?}ÚW\Wί?èe{³ÌÓ?À#EªY/q?ÍÂÿ·ŽTË?¿ôwek?HÆC"?{€7ÎC‰ˆ?í µÊ¢?¡vâéÒh®?±˗©»Œ? r݅¼?8¡UM•?$EINÀ9ç?ê½âÑØ?¢÷㴗b7?Äÿ/Ët³?¢óF}ûžëPSR4FGL J1105.4-6108?¸ï••ý"˜¿ë˜<8dÀ8°8\gßãÀ:â¤itš@È(MQ@eº|h0k?»ÈÉ2
™F?Ôō]¡í@Y:´0ô•?ûÓÒ¥~Õ?ëtž½ÅÈͿӌÎû%OÆ¿ãê™fmó#¿çÔoŽ-TÍ¿ë€<01öó¿ïÿþ½à ¿PSRPSR3FGL J1105.2-6113PSR J1105-6107?ßߘP¼?/•XÆ?ì"» ÷Ô/?Ä(˜Ò–²¬?ºî'«ßu?ÄÂÁÊÕ?¡Óî
Á?¢Án-†Ö0?Û\FØ+¥ ?À–•Î]ñx?á4²òŸß?Àm¨¯­?´Gô{s†
?£~(¯`3?åcêÏÛå?´í7ÅK÷?ÐÕ;
Âü"?±'ù2ù?"qû¬Š&?q¼[ô-S?âòYó«!Æ?­«–Teˆ?Øä,^q"1?­¹Ž'ip??†Ÿ"àù¬3?'£)?÷_?ì¦~'ÖV¹?»Õ" ƒ?·ø'vF²?º£ÈJö¸?ƒõãÛªà½?‰öãLƒ?ßoÊÉùný?Æüëòñ"o?ßð†»?ÆÁ©µp?¢ñÇP]¦Ô?•ŸŸ×œ»?çä]pR›?³ÌÐÂi‹N?˲ò^EŸ?²2¨aÈç?i°JÊ_§?Q[ÈÂÂØæ?åsWoÊà†?´ 2gñ?ÔåððB´?´e<½MIXED4FGL J1111.8-6039¿Ú©=ó$ó¿¼$(ÿ'½ßÀ7—V¸sytÀ:'o™ëÎñ@ <|k‹iU@ËŲý?§hìÁ?Õgùä]K@*ß¼@ùý‡?åEfîVŠ¿ØÌï,¿Ø>("®zý¿ßw»B¶³Ü¿éêœ÷+°¿í'T·PSRPSR3FGL J1111.9-6038PSR J1111-6039?`ôðZƒÂ?^èÑ0Mìm?îFÖI¶?¨î¿eÛüë?ªƒLhGîÕ?¨Wݾ1?vÑýÏ~Kî?…7ÄQ#?ç…dD'ï?½³I:}÷Ÿ?ЙïÕ"\?½ÐjjpÐç?¨bò‡7Y?Ÿ¹X$$¸?èF´(ê¶?²º¡yu?ÈÌr»D T?°àóÊbpU?XêBÌÖÏY?EŸ|,·#?å¬òI^ã?¬>¥ó"6Þ?ԍ1+qù?¬3ÛAEê?j¨ºô³Ê?ekWpæT?힜"§šÂ?­$Òð˜Ò÷?²5Ջ'?¬*Ù¡¶7y?rŸôOé9y?z "N ÿÄ?è*cb>Ó>?Ãñ,
á%[?ÎÁrÓ©'<?Ãíd÷bÒ? ahu–La?™¶I)sÿ?é.pÑNfÀ?´K¦3R_@?Ç-âœ÷h?±Þ	?0ék¸˜f¶?$zµ4}Þv?æ¼³øÝø?°!®*Q5?҂_œ®Þ?° †èyìúPSR4FGL J1112.1-6108¿ãw/L¿á8­€¬7×À8•nÛí÷À:g µí7@ DØÒ³'@¨^=¢ø¾?ƪ^û'?Ͳ 8¯žê@RÎ-±ê?ñk	Ãù¨¿ê `þG™?ïKÄúpt¿çcÅ×惿ãíNL"-I¿ìTA ´@¿àÀ*ݤ5PSRPSR2FGL J1112.5-6105PSR J1112-6103?—$Hü̃w? ¯^­ÙnP?ß
ófȳ?ÚVñ6l+U?߂ȏ=?هç+.H?›©6ã;â?¤Ñú¸\A8?҃±I[á?Âg)7k÷?åàÝÉQö ?Áà [ë
U?·:w\±Eƒ?¢IŽæΆ?Éf`éò?°dç˜ý}Ê?æ¿ÚŒ^?²ÆñãÔô?‰›[:¹9r?joY0
ª?Ö£'2?®£Š´#‰?ä'@ÊÔÓ?­óHÇѾ?£Ä(rì°?¥.õpµ÷?Òc"e;)]?ѹÿtX±6?åœQŠ¿¿§?Ò¢_çØR"?‰Õ¹Eáš?"4І©r?Ó»»Ç/Ä?ÆBxíÉéæ?åØË<÷#°?ÅàÑÇ¢/?²ò¥·O±?œŠšeU÷?Ì¢]U¤)ô?²9g«)?æ"êUÒM?³gR¦iV?eÓN´'–E?Pº¥'x€?فžè°O‹?·V!LÓX²?ã)]<Ø3Ä?·JC˜eOTHER4FGL J1119.1-6127¿ïúû܄е¿áv"Ž¾À7܉ð¯*%À:ÀY‰QÞ@iœÄò7ë@J<d4]?¨ZàÜò?Å­7Ü_ï@;ÕýÍö˜@È¡Îï?âèˆ6ê?Ôkf€g™l¿ânE1by¿äärp_äl¿éBpˆ(X¿âÕð'3¡mPSRPSR3FGL J1119.1-6127PSR J1119-6127?·kÓ-ê?±pvWã?ÒDÑ'œÉq?È>ÒJK?ãðK¶?Èî& Ô?¦<®z.øÄ?«"jÈÏt?ÖéÔêþf"?ÄùOp?ã'J¢™%3?Å7–uø«?҇àe@o?²Ñí-"…?ÄþÖïTP?«"ßzÃMo?á|ˆW¹
´?µW«çP»í?»ô^:Œ²š?"탚Œ…J?Ù{:·°•?¨÷œÞacŒ?߇­ºI"Å?¨sÚØ©#û?¨€²—Ñ5?L4ÍAZÌ?Ó$'©O?Ä¡àè-.?äå¬ìˆC?ĽÁ¿Ü&?"v若Ý?™´[ hÿi?Ôîwӗ?Ê®±fSF?äå>ÌL&þ?ÊÄ»¤dŽ?Æ¢gØp2Ý?°Ù+Z×$?ÇF6`å?°ð/|^9?ä…å¼Kº?µzê|T3?ž 4ö#T»?€z%û:{?ÞõÎøâû?²z¶ÿŠr?ß(-·"wZ?²9ñʽeíOTHER4FGL J1124.0-3653?Ês	†€Q
@6ÁÁBá&À9#ˆ©[®À<JDÇ°-@óG;¨Í"?þOU!š"?¯Õ?Pç"?ÕÄ C@%dBAÃï®@¿é³¸SÄ?ïÿQŸ/пÊ
Þdú«'¿Ú¸©>Ó$€¿á'Þl	¿íR«ž~Ü¿ïûªÐù'7PSRPSR3FGL J1123.9-3653PSR J1124-3653?–í#Ž¸Zž?ãbAfóA?îJe²iý¨?¤E~S0îN?ŸÆ&"P"\?œµûàØë?˜~ÈáDxâ?™s'‹í»X?í—gî¯SH?©å=·­?ªJ¤h?£:f'X?¡)Â8wªV?˜Ö¹Ž'?éÓ°æ´¡Õ?°óîF;›?ÄfË×ëu?®""Щg?¬`RKãiƒ?»"Öð?êûÿ¥ÿÑ?šà¡4ð,?¹ïÝ⸋;?"Å`¬K>?œÂ®x¿R'?'Û®Bò8¯?íĔˆHõx?§a«'tÏ?¥U`@ÈÍ-? ¶¤œ¡]?ŠÐpăë?'§wV7j?î%^̜¯?¨î"h!áÙ?¦ûmâ:M?¥jZɜŽ
?'=3‡Ùã?‹¾ð@Dh»?ê̈W/šU?²;
gå?†80üË?±ëà™ã_n?'ËlΫk?{ÁŽÙã½Õ?ëÖô_?œç"TpÂ?¼Ü=(æR?šùÖyPSR4FGL J1124.7-5915¿ï¾–8f"õ?ü;V¸sytÀ7"^±f>ùÀ;ÔoX}p@!õÅ¿g_@_Á}ä1?!§"Kâà?ÎêõVÙ«'@(y!S6ß@-¨ìô-¿Ç®†»›w¿Üf9e&u`¿ä0&8xí¿èöÚQðœ¿ìÄw…¿ä®ÑnòüâPSRPSR3FGL J1124.5-5915PSR J1124-5916?—iàÒì\?šÝv×çvá?ésÏÔ=?ƹ|¸ã5ð?ÇFD¥ÿâ?Ħh
tK›?ŠYõ©_Á? Ãt+?è²ÚlêÜO?¾õ"¼gÏÈ?˔€­0ò‰?¿T}\ø?Á¼|-ß—?ªp'Ó§s?ã~ßò‹½?³öƒ7åM?Ð$Ìy|?±ÛX‹i­?~.,ïÿ?hRZ4趬?ëÉÍ?¨%g? #VìÒ¥?¿Î³A`r‡?ŸžO°2?ˆo'2X/?"wÍ=IZg?êù\þÍ?»vŸñM?''®ÒÇ?¹vÑÉüõ?ˆ1ša'¨µ?®‹Û
˜®?éôí)?Æ0Ȫ~CR?Êi¦~b?ĵÖíºÈ?°[
:1"d? ºïSú?å³.Q]Pú?¶à·6‹Íì?ЂàÎ(4?³|,ªO[?YcÆƜà¸?Iò&yÝô!?ì%Ã÷ø0?¤÷"Šê5[?¾qºÇ*;?¤Ý-nØbÉPSR4FGL J1125.6-5825¿î°mJ[@À¥º9LRÀ9׋œ€ÕÀ<T›ñb®@ )c:âÔ÷@CüäŒØ?Àž":ê?᏾ˆfk@­'"ª?÷«]ƒé¯¿Ï"'ª>˜?ǗOýÄ;"¿Êµ_]]©)¿ÚHE¾ûþ¿¿íŒ*¢k¿ïÿ¬óéqHPSRPSR3FGL J1125.3-5824PSR J1125-5825?'[±ÆOôÏ?'OH^éo?îò®øjN?¨—/."7?¥Bü1œã¯?¢mœ˜U
™?‹Õ!ě±ê?•ªI~ÉëŽ?æ‰Ìûyf&?Åûpñ|&?Ò
¼úzb¥?Å[W=¤ž?³S®Ïßò\?¡ÏßAg«?éY»Î€^¾?¬«¨üî:¡?Àï9^E…›?¦}eΔb?¬Ð:‹.V?‹Nzmà?ë/ø+RòŸ?¢‡dË¢#ƒ?¸vֆØù`? ãgþ¡C?~cyX"Ú4?w@úÈØQ?îqQv•2­?£2ød{
Õ?¥ylmo?¡4ý»;±°?Ê6Q™"m?•¸rv	ߌ?åç©:È?ÍJbã
?Ó²ŸÔ5Æ?ÍŒ)L2;?¤ów'(Êá?š`I·q*l?ë
S|)?®Ä87U¶ÿ?½§T±÷Î?¨lI̟"?†1PÚãæÅ?qð™`ÞÄö?íš",{?£ZBU_äß?´ýKDÏ?¢ºøl–^ÚPSR4FGL J1126.4-6011¿í­Ñ\ÝY?îÅ2@QÀ:"ä;~[PÀ<?‰öŽg6@j­b#`­@Êþ§°´?ÑGAˆ
¦?æ²uhaé)@¤X9|ùP?ü÷s¼»1Å¿ïÿcW¾,÷?ïý(IË%-¿âÖ斢nT¿ác¿ø¨óª¿ïÿÙi"A'¿Õ›Ä¡Û¡PSRPSR3FGL J1125.6-6012PSR J1125-6014?à>ÀÅë?Äuésú?Êÿ4:?ºû)}8 >?ҁ\,Œâ?öÌ|½7P?®L>‰2I?´¥?\dÄ?Ñ*R§ K?ÃS¹ê¶±q?å†Ãs ?ÄÎëIx^?ãø™Ñš3?´	r)õ8?Àe;ÝÀ~Ð?¦q,PŸÿ?џpÝ|Œ1?°–/Ô²^?Ќ
eªdÿ?§#Šç­¬T?âºÔO«—|?°OyԜ?Ãü"ø"™'?§äÚo)?ÔìyÈ:cK?Â]
Œ°}?Ôò-?˔?Ãc6½ù—¨?Ö!n
…Ñ!?Å7¬äþN?žòD۔¸?¦aÈ¢Àà?Ö"þæ-?̊L¹ZîÓ?ãù_΂ë"?̒ÞÎp՚?Û¼ÖÉê‰?µ6¡	¢¡?Ç€3äUw?¬c¨wR_?Ø¿i#L5?´"
¨»é?®…ѽVË?"íÁBŸ]?èq!!Q£%?´^õP³þs?Ƶš¸:?³_Ÿ™ÃMIXED4FGL J1135.2-6055?°©Ë p'?Ⱃ`št‹À7Ð*o?RüÀ;4Ôóâ»@'±«^="@+¯EÓHè?¢XèàÞk?Ò<(…a9@&é䒼/Ç@>óp-?Ó3ÊnJ¶¿×M†00It¿áõÖ±R¿æà@è'œ&¿îiΛ&%¿ä±úƒ¿<ÁPSRPSR3FGL J1135.2-6054PSR J1135-6055?j0PÁºF?nåô5¦eê?íÂ9€ Ä?²¦u_:"ž?±±zēÚ?²gôÕÜ>P?†Z™ìŠ3H?W
zmµ?èÔH¤'?¸6é"q™?ËI4\(?¸Xb°÷±?£Wc¬1S?šßÍÓÕL?뀕Šâ®?¨\@7+$?º:««¬g?£w|_0™?|G(¤·?c·~
ä¶×?ì"7blÝ?›·ð&+(q?½ÎμO?›…Å|K€?gåóÂãs?e¶^€¦Éý?î@çϐ)6?£{eW™?ª€4¦wcê?¢¿@Âçù?{UWc•?">šj[â?èþEfw6?Á{~žÒ¥?Ë,BځQŠ?Á`8ÏÕ?ã?Œ•óäíº?‹
ª‹«Û–?ìÄ@ðÕ£?§R(ûMž?¶K:ñqì?¤êÅˈ?U&ùnä_Ì?D0d8⁧?ìžQcÂ>¡?Ÿä¸á9i¤?º¸Øú¹>?ŸÒ»Q>tPSR4FGL J1137.6+7527¿ï§²"z"@DeìÃã?À<ÝLvÑÀ=ž™Ó{<·@ ,Õöí@dÀĀÍñ?Õ¨ß<ÿí?æ÷]ßÚ¾@
Dr¦É¢?øçý%	O¿ï–­94?ïÿ—Yοо­dҒŠ¿ßv•¾BÆN¿ïÿ¹‰#)Ñ?·%—"0ÏPSRPSR3FGL J1136.1+7523PSR J1137+7528?êpc?Â1ÓjS?ę¸1y
¢?ÁÃb¼sõV?›$,zÊ[	?—:¾Sš?ߑJr6uª?ÊHÁ¿o?Ú†ESò?ÉcA݉Í8?¹|½!Ö`í?©=ÀÂÞ?åÂáÕ%>‡?²©ÒÇ+°Ú?ÃØj˜WÙ?ªçôG=–?Åñ >¬ì?«½?æÛæ?àJ¨Ìג?±¨Ôé—Ã?Ýf÷Áÿ$Ÿ?°ìÂ#þY? ¿îíÞë?–~EÛJvÃ?èuâyÿ—È?Ã:®/[jè?ɔw¹Ó~u?¤JÇgz?¢Oùy"p¯?›ÔÃ?Îñdûµ?ǁÎïXa?ã"'^´8?۝8pÅ÷?ÂþhRq3k?»Å{_?â{ZX)üm?µU¥/'?Èe×ö ®?±ÀïM«"?Íû0Çaí ?±ÃÙÞ(÷?ÆQÓ¥a¬v?«'3Ó?xS?èˆèþ sA?²qß-†ý´?®*!}Þe?¦[Þ:A÷MIXED4FGL J1142.8+0120¿ì,tÓ´@Mµ\î À9Î{€©Þ‹À<F@îݘÍ@=5?§á?úñўå?¹Å‡Gw8?ՆhD7@P<«ù@ëpTü±—?ߟy'wéñ¿ÒcÀ"?h¿ÒTÑ]Ö¿ßÛAÖNV¿ëêòòÑCT¿è:"DÇPSRPSR3FGL J1142.9+0120PSR J1142+0119?ÁÜGQ€Ù¸?·W"N'î?êCÛÒNA?¼Ìþ
‡mr?¤Q%™d?ŸžÆOP´?Ô"¤æåãÛ?ÅÓ÷Áö™?âpÄcÐ<¡?ƌ³¢Y[¼?»ïIE拇?±»¼ ƒ
~?Åå~xŨZ?®³¯?ç(¡.A?³%.¼¿?ºô¦×?¥°¬ÙÝï?àKx†E÷(?«ÖCÿ'?Ó;àß[ù?«çsÖá?ȹ¦#©ò?¡ä,Ž(?³90D¸¹?¦Ÿ#œ<a/?ì2…|í˜?±~Èý?»?¦eG··'\? UR¹"r?ÃǍ
Ö= ?ÂÄx%³?çÜÚÈN?Çq:ˆo®A?¼aÿ'T?µ9'X!Ž¢?¶V³zr5G?¥°C
͜?êX{Õ72?­}E÷—6ú?¶åsÏR§?£³=1HST?ҘÅ
ƒ*?«²§?ÙO-ôž½?µf·žÄ$'?ԫLjY?±=ey¾MIXED4FGL J1152.0-6107?ëÈ$W´X?íwƒßóðþÀ95èºiúÀ;£ã³™ @XZÂnO@±æ­j1?¹œ÷rë:?سµÄÈqs@™eéŠs@HÑQkØ?èÎ{·?ïÚ&ò³c¿áªjÂkŸá¿çQ.ƼèS¿ï
¸Á?Èñ:j_kPSRPSR3FGL J1151.8-6108PSR J1151-6108?ºúB]¿ñ?°ÝkU»?çÀC"
õr?Ág;Ýj˜"?ÁЄè1­?¸ES'oB?¯W!¸­??ºNHÔ¨R?á63_Ë9?Éáï*½b?Ù¨µ	¦`Á?Èٛ&âlò?ÃEs–i}?«/P.ÿb?â/QÐ	ö¬?´w¤eö5?Ñß¹§3¾§?°HñÛUúÔ?¾.VÕyĒ?›Ò™änßD?çÒ0Td8í?¬_à™ÁV?Á C²:?¤ÔoRß{?¤ÃQà%"?•¿W×?êˆ~ÿüf?»d;åo—#?À­@.]$b?¶·sÅVˆ?'ː´.—?£FOkh¨?âC‡Z%?Θ8Þa¿?Ùпæ_oý?ÎI	Ô®?³=	CJ¿? ù™5y(?ätqØp«?¹2õT88?ÒGÙþŽÒ?¶@9Ö
o7?›—òþÏN=?"˜—$?ë3ž'°O?«`Óãï?¿¾N¸Ru?¨²[š*PSR4FGL J1207.4-5050?ë)B2´'@&՚•BÀ:Ô©: À<€`mþá@M˜f"³@ˆÌ»ÑÓ?¿Úø‰"ò?䂓=_ @E"¼»Ò@»ž`²?ë­2h2?ïÆÖÖ¿Õ^ü· =¿åÜá­¿îXO·Î8¿ïÿ™"{UPSRPSR3FGL J1207.2-5052PSR J1207-5050?"´/‹Í—è?"]{YÜ?ï$D¸–´ã?˜5¤èÝBŸ?{ål±ÿ?{¥àŽÈr²?¥¨µÒp‹ê?©­t-S"4?ë:s¸xEÑ?»jÍ[ñ?»XS‹…?¶tÿ³v[ô?¾!ß<ªÄÿ?§]Y'‡°?éÍ«þ\M?¬Ì mF ?³pÀѼ¬¶? 9WpO)?¹­5¾äé?š‹pÙSe?ëjBw…ð? äIÑ|ê?¦ ~V 2?"¯ò€Îb?ª¬CnÚs?ƒ60§áZ¡?ï‹ò"Wÿ×?ŽèՀQS?v±–iÿ6?zÇÔf[k?–ï½tø×? ã^®'ù7?ëü´ÖƒQP?½ëËÐoç?º^jt'M?»j»Â…Ãp?¤Ù!µUŽ‡?™Lޑ+#?ìÎr•Z
?¢æ˜nÙùò?®?´÷ž%¨?™ÿ™¯'J?˜vWº.Ã?ƒLXè3é?íÿMfvgÌ?™_#W?£Ð"qîÑ?"'$ãã_xPSR4FGL J1208.2-6237¿ìž§ ö㪿Ʃ¸J´¯À7ýùp™ÆÀ:'Ӂô@ùx}À?@'í»YÝÂ?°jýNõ±r?Сzäw¹J@ ™íZáÍæ?ÿÏ懳é¿íå`³I?îïV.྿ãäÅø¿ä9€ô¿ì[`®–€à¿ì•†z$PSRPSR3FGL J1208.4-6239PSR J1208-6238?zå~XMY‡?ƒfmiV«?ï	»¾~?¥—'gH'n?™Ei•)â?¡êC±(Ù?‰î7
H5?<'û5?åMeàžT®?ÁÝ)ÄÓ?ԕ†Å#?Àè1ì>á?°(ëjˆ?ŸáŸ—µhØ?æ"'¢mcí?°à:¢²)Û?Ïaçð??®yCÛôs_?€ü& ‹x?e´?eX8?åàpSá:?¯G\Çío#?ÕU¿??¯
xŽ‡à?jh=ñÈÓ?fË|Ù°&?ï«£SÏ?gLaÏË?š]ƒÛð•Ð?›}á¢|)?u$L½ª?~\áæc£?æþç7r?ÅÚ­!Ù?Ñ­¡kþ‰f?ÅȜ½i?Ÿ‹ÒÙ·F?•xPÙSµ?èÅUٕ þ?²Sê?§ÊZ?Èù.?-'_?°Ç\Ü#‡?Vü¿Ó0?D5]ç&ó?çIA@M^>?³.÷ÎÖ?ÑV€¿øô?³(3­ÿPSR4FGL J1221.4-0634?èËF=¸-•@KÂFŸ¸À9Ûò¿¥œÝÀ<E¿çáü	@îFïÿ@‡ü¹#£?¹_ !·"?ÕîžÄ%ß8@0T9=@dø7^»ø¿Öǁ¿gR¿ÖÌP:ªö¹¿Þ²«£Ý?a¿å{ºÁ1Ž¿îPüD‰¿ÂVjoàb¬PSRPSR3FGL J1221.5-0632PSR J1221-0633?Ô= dd´?Æá¬ÍþÑ?ãdšth@?ÊÃäÍ/ÚI?³äªÉs¥4?¬u¨QÑ?à¡¡Z®!f?Ép×I5?×á'OÚD?ÇúšÈ:8X?»nÚåO‹À?­(Ÿž1x?Îl_œ@?³‡¿ÌÓ¯?ä'6úp§'?¶9¥­Âÿ?¿EomBšý?¤F¿T"µ´?çó…ð^;8?¢²¦‰UÏv?Å6€ÁAºq? :(V¦¶?µöÎþh@Õ?ŽS¾C<¿?ÀÓ±‡IF?´¾qŠôË?é*€ÿf?¼›‡3Õ3g?µ·ôžY=?ªâÅÖY+?Ðdôr~ô?ÇÊ&K»?ã¤v€K%)?ÉÝjh9?À¤=¬mv?¶:Ñw>ko?¹Ã£) ›è?¦Ç v©:Þ?é!›ƒ?±H;í'Ê?¾3›Ê°?¦8"·å?ßÝaHßÎ?°%}Ïó?Ô_\vN?°Ôa¨9æ?dž"10,K?£AJn«\ÏMIXED4FGL J1228.0-4853¿ë¶äªRé @+Hˆ/À8ƒ—‰!SÀ;gFvš@ÛýlR@,M€¼S?¦|)`y	?ÉDã^߉@rT¶"¥@<Y¹YÓ[?ï®K75÷3¿æ4€ãÀ.¿âb·O
¿å¢•Ä¿êá,À¨QB¿ïÿ}ß(ïãPSRPSR3FGL J1227.9-4854PSR J1227-4853?1G
?«eæI+µ>?¡Šùowo?ªª"«`t?‡°Mìñ%4?|Ç÷v–?æؒяµ?ÐQ92ü›?Ƴ^‹å¸?ɆVĐpÚ?»Ô­Ê[¶é?¼Õu¤Ö?ëÇ~s^?­:ªÒ¥I"?¹Ú"Ãé³?§ññUŠy€?ªßB"Pä²?œ#O'¢›Ç?åBOþ?­ÇÜ°½x?Ã6°-ü?¢`}¸h?ȘF»Ù¾?¦÷Wa|!?ìä0½H[ ?±Æ°ÄnJ?µ<–ÂÑU°?±K'Ê°?‰Ÿú§?‡@®ÒÙÑ?áðlà0µ]?ÒoÆb‹¡›?ÐÇLoÅ4Ó?ÐfPìׄ6?Ư³Ÿ²Àæ?Ä¥‡¨DF?藷d/Õ[?±"Nƒ¨?Å=_øÊ<á?¯^²wgê?°Ç"ì~çé? *£It&é?Ӂ[ˆ?®~´ˆTÅ!?ՙ'W³›#?±¦Py¼šÖ?Öå" 2ÇË?´yª_fMIXED4FGL J1231.1-1412?ï3¥-˜áÛ@H0!¼jÀ7[ñ˜^À;WÔGëQ@Ú¸æ;é?ù—¡øìx?"äùБ?Ûü}¿sré@G1ïÝëÙ@	÷ï†á>?Ô½C¢—7?š¤^ˆeXŽ¿ÔŒËÀ]RÁ¿ã†€¸!D¿íîˆwÆ¿ïÿÿ&¦³PSRPSR3FGL J1231.2-1411PSR J1231-1411?®VÅîÞ±?µèᚖ$?í®%@<—F?»rª3Ū?‹|æÝ#š?©‹8ež«¬?…ÿœCGFs?¤È ­¯3?î×¼-ÜöÕ?²åÎrá–?š¬)œº?©·ë¿+N?ÁO
[¤ó?ªz!vu¼À?ç`™•N?²ÃW(~ûé?Á0Œ>+"²?¬5+úŒ°>Q8XAý.o>dÐ,ñù¿?ïøŽ••º"?P|7Ԛ°ø?MŇ¿Y ?P|)Sõ?µc!1"Û'?¶
	½hã?ìÙ
.ß?º.Œ
¦²?Ž£ªÂöZ? ùúÞQ0T?‡¹3 'óg?©9µ0‹Ž?îyäµG—?À°mÃIc?¢sgÃû?½BÂXËü?½9uv­9?¨À
è('\?èD wCÙ?³Ü
!Áñ§?ÀSCg™þ?®Ýv]n‹>:±è¯T×D>`MlHcË?ïèî–v#ž?t>č@v?gf0=æè?t=pnçPSR4FGL J1253.3-5816¿—&JA—¤ø@Y˜*ŽÀ:0%™È"À<
9¶Úó@Z¾bѱc@C'ŸÐ€?Ó ¡ ¤%?鍺}¿ÉY@
}œãÐõ@ÀÁ­§n?ëˆGô·M¿·á(V¶E¿éü…%Ä¿êÍñŪ™œ¿ð?ïÿüÉï£PSRpsrPSR J1253-5820?æjÕ³ž-?Äz 8bP?ÁìàÓêÎ@?½;L\OV?ÄgÈ]ž¹?¾ô°6?ÙC"N®¹¼?Ìndj@n8?ͦï>Lýñ?Âj¬Nۍã?×é*ÇK?Æâ3!¦ª
?â¼c¢ß
	?²¥áêTíÏ?ÂrXsÈz?¦cçé°H¸?ÑN¹ˆ²?¯Dzê¥?ßÂti^hk?²[k»@܊?ØU´i úÙ?±½³¯ch,?¿Ÿ\´rî?Ÿðò"RO%?âS"ãµü?É50ʉb?ÌÁh¯@ö?Åoøz>yQ?Éð¨
íç?ÃEèf2?ý1@?ÅfÝØko?ØìÉn¯
?Êlö¡:*|?݃Xwîח?ʍ™ü@ù?ٜö¾Ï?³FðfÞE?ÌZ	–·%?²@_­Äܯ?Ø6y>/ež?´"Ë|á??Â!±'»Óù?ª–8!jÅ?åVðŒ<a?¸»üÉ?ȂŒLTƒ?±kæì;Z¨MIXED4FGL J1301.6+0834¿ïd&}ÀÚ@Q҄ßÎ1QÀ9¨b/ ¼À<[å¯ò¡s@íJÛp~˜?þÚÙÕÉˑ?µ`J~ºW?ÚLó£¦7ã@ ÇTŸ"…^@^¨¯à?ÓÙp^·ÆU¿ÉÉ<Ê`¶Ï¿Ý"€ÐÊÞ¿å£ü~Á&&¿ï
ý˜F³¿ïÿ±[W>«PSRPSR3FGL J1301.6+0832PSR J1301+0833?Ÿ˜×Vϒ? <o؁Ó?ôå£;?¤[ózCdš?Œî"8f?ˆsy͵û±?Ä´äxºý?Ƈ6ŒüI´?腞•àZ&?È•ôQ(Å?³¹¡‹{TÒ?¯F»6ˆŽk?¼û(%£9?¨L	0êÔV?é$/ýï¸?¯
$O4?¹ã[ëŸ\
?¤ù¿$;Ë=?Ð(J|Pª?©?áâö"M?äƒÇOµIù?­RùÍæò ?»@›''?˜äm¨O?žT˼ßøV?"èôb–b?îimô>°? ‰9qˆ%?"}u¾Ìm§?ŒÐ3y€?±°UÞ-ó-?¼Wºžnb?ëXŠ94ï?ÂtúÓ_'?³‹V(e]?²¼âxª?­€`×{¤? <o‰/&$?ëº3˜?¬ Îò4óú?¸ÏG»hfë?¦,UèÀ?·÷¸Ñ?Æ?žÎÏXÑ?èjýÙ#?¯_©óSÖ?ÁŽ{ÁŸû'?¥Tùõ\µPSR4FGL J1302.4-3258¿äŸ… '/ß@=ØOãm"BÀ9>³"&jÎÀ</#qõâ@¬–"¨q?ú£2ü¬Ž?´ä!s€?áì(¢‹…°@(žZWdjä?ò–"VŽ­¿ÖZE›ÀS¿Ä½¯¸ê¬¿É€Äápó³¿à%°"±"L¿ít0Ôý¿ïþ/{ÎSPSRPSR3FGL J1302.3-3259PSR J1302-3258?…$'‰ï}]?‹Ê€îÝ*Ù?îíπ8ï?°äX!oµq?—³Æ³±‡r?®Ï×ïð²=?‰•uš!Y
?"¤êRÀ?î†,"Ë"+?£iÿP—B?¡7Ù[©?æݺÈÍÁ?¡ ïNVû?™,KAÚ±`?êR±·‡Ž?²‰bÛ¨˜÷?ÂM%Œ#?±02	j÷k?x¿º'?bî1Óäýq?큯&7'?—3±ã[gV?²p¥"ÿ¥?–BˆÉdMâ?È`ÚÊâ?ڋöD ?îûÈîúQÉ?¡[…z½[L?'¢±¬qá?—HÆ–¯?ƒ!S^zú?ŒPçrAEX?îÆgŠu0Ñ?¡›:$0d`?¢dïBîg?œÛ¦'«Ù?™]ÿÙwQ±?•¹oÊS¥ã?ë$ÿ‹2?°m²Ýæº/?½@NàÉë?­ð(ûÚ}ü?\ӘKAn?Léƒ÷F¨?í[L¯ž?ŸýÓ®RB?´²Q1ß?Ÿ'Õ˜ùBPSR4FGL J1304.4+1203?ä¼TL»øó@R¨¬1'À;cجëÀ<ñI{t¥@?Ž7£@2[úҙ•?Ï}$"®?ïfAý{k@<o"͊b?üw­ñ•Y¿êÕ>¶I(¿à»J>³‡¿ÁW)‡Óh¿ëìÀ|ÝK¿ïÿ>ñØJ?àæ.¢=PSRpsr3FGL J1304.6+1200PSR J1304+12?Ï?óLµ²¡?ƌ'øF÷?ãë_‰tÕ·?Í3V•¡E?ÁŽvö?º&_Áu?Á"†`'øý?ÁÀæ5dÌï?é2upøï?ĵAjÈ?³EG¶¤¡?°Þ-¸Ä?Ò —
?²—miÙÆ,?â~[šQò³?´`j˜¸
Ç?ÀÅc·ât?¥hr£>;®?Í90¤ô¨?±½µÁÑË?榀‡Ï ?³´Ý™ðùÊ?°YÑ_Ê-?™îkznÓj?±gÝpT?¸*Úß @?äœ
ÙçH?ÇÕ

<fZ?ÊÞlºñá?Ã
ì&Ú4i?±iRÄÿì?¾Šx"fSò?뭈²IFy?ÂÜw£V¥?±*g©ÿº­?³!í`åÝ?ƌ€t#G?°&•Û'ñ?æ	ïñÀß?µ¤Ø¬æ?ÁK¿É%š¼?§óC¦?«dÍée0r?™ŽPÔó{§?ëÅ=»')ø?­[ü»^Á?´#«/Ÿÿ?¥WׯS§PSR4FGL J1306.8-4035¿Ëi¨ê5@6-gý?[`À9wòŽþ5%À;ܱ?¨Œ|@­•£•ÆÑ@ìgßã*?µÉɍ'Ei?Ãð˜Ä\Ð@¯Ê]†ÃÔ@ZMxß?ï÷¡!MW¢¿á‰Óˆ¨°Ž¿ä{=ï홿ãX)Âq)8¿ïÿø]Ê5™?Ø®'úîôPSRpsr3FGL J1306.8-4031PSR J1306-4035?í~Ïÿº¾`?§I"'à?›õ
˹f?˜DSü]\r?ªzŸSMø?Ÿ9÷…y?ê.øVq?ź5ô¯?¾
æü?Ásêë=G¬?°i'=µù?«d´H¥?ëðÁõêd?¨ÀO
tÖÃ?®´·­*ðï? ÃCÓ¥ ?±%.ßMm?r@fø¿?ëðڜcI?"ÁCzÕ¾?¨—@S FC?‡:(¾?´-ŠóP©˜?tÍPcf?ép ÿê?¼+–ÔØ?¹…ä"ÅJú?²š4(Ž…
?½¾šçÄÂ4?³øu ?æÌɜÁ—?Ê͈"8±¢?ǂ& ÓŸ¥?Ç«v)Á´?¼}Lqr³ý?´äoÊ õ?çÍã8Q³¯?±1ü(§`y?½z"¤DöÞ?¨yØl¿Ñ$?Â(̖µÓ?§"27ºË?ænÿgª?©ãñÔ§ô?¼"þ²ÖŠ?¡Ö–õY?Çýv—M?¥©[úçAGN4FGL J1311.7-3430?ïoËgG@<,Š›ÏÔ¿À7…H-–;@À;fDH.lû@̓j5©@X²éÌ·Ô?˜¨yÜ9ý'?É!@ûBV@0 À~á@Ü4ÌesÍ¿›÷ý8`ªÌ¿ÚºìDâ2:¿âp·ù1¿ä²tË•¿ìËLd\ ë¿ëˆG◺FPSRPSR3FGL J1311.8-3430PSR J1311-3430?ÐcŒ^?¿ÕË	d?ِ¯{?Ðýéû0ã?֚ãù²>?ÆöŠ(•þã?¹©S,ð|?ÉX<ŒÎ/#?êxCÀôýC?Îñn0£ûŒ?²"ŽÌ±Õî?¶ÛL"tG?Ôç֍ÍÚ?µ¤6‡çŖ?àÞà~8?¸CCՍ}¼?Åì×cÿƒÙ?®þ²)Ól?}.½"è?pw£"K?íÜa%þ?•H£vã?®"	0?"VÚ'4i˜?Á#Æfùš?¹åBºdÀI?äpÙfçÁ?ÊÑÜ<g ‰?ÍÕrýgc?¯P?¶!ú•P?È—§¯ƒ?ê瀴½®Ä?ФOý»¤~?²¢S¡?¾xk·?j?ÍRýö1í?´1âžlÓm?â`Ž&/$í?¹ª´€òü?É|tiM:_?±äfô
?ccÒ$Å?]¢àúQv?íy[R$ÿ®?¡få à?³šÞJák? õÆt¦ÂPSR4FGL J1312.7+0050?éž‹6@Oœ1&éxÕÀ8ö6êÀ;øždÚu,@Öþ~ö€$@ŒÏkã}é?®>—?w9G?ßBÚ$ú
s@,mXê|àü@́±ñTA?æêZ±ý=®¿Ã)Ê(ؑQ¿ÚæÝR¿æAP—ÈB¿î釃 U¿ïû	h^ŽPSRPSR3FGL J1312.7+0051PSR J1312+0051?yð¦"w?w'è4eB?ïSh۔Cw?š6X9y‰´?Ž£¾ª'òz?–Ác'?•ê?˜Óß2!‡²?ª}üÇE·5?íôêÃWÙ?±o'`®EÂ?¤Gd-&(ß?¤Fƒ²Ï?¥¾v?CÚ? Öõ$v£?쓶Æ{$?§^ΣƒÖ£?°ƒ«©‰? ¦˜€uùZ?pBkdóä°?]‡Äن,?îóØÃÒ ?…5Ã:º¬ˆ?tLÄXþØ?"5§®ƒ¡?vÈÞ­TI?z?0ÊQ¸$?ï\£^im?•åÓ\ð?¯²©˜¼»?˜³½°¯?ŽN=7‡?–
üè†W?îSòNF+?«@*"V¨f?£-KØ9 1?¥4ŽÊU±?šýxnÚ0ì?˜è~æT¨?íi4=ŽÍ?¡ðŸ84¼Û?«íÿòDÿ¯?œw¼TM—à?JTۊß™?>24õ?ï´)½¾'?ˆßè#
£?žvÓêúê?‡ÌÈ(õ®PSR4FGL J1335.0-5656?á?ÝR@­µR\Ä&À9œVwÛÙ°À;ÞIWaç@``LpñÛ?þÊﲪâ—?¿ç¾€-â¼?ÚÓíNL"@^aIÆóo?ù;¬Îª?Ä|*ˆiÆm¿ãUeÂÒx¿ÖT¾\‡¿à£v'id¿í¼<e›:¿ïÿ¶Ï4†PSRpsr3FGL J1335.1-5655PSR J1335-5656?«Êÿ㽏?ªŽ.|KGU?ë:Pí>˜}?½x¼Ù~zÉ?¸^"‡PÎ?´/é	–?°†~¿æ™Ù?²¹rÇB«>?ãzëx^‹?Åþ'§d³?Ôê$x§¨ó?Ü[¼z€`?ºVXãW9?¥Ìõ57?çYH€v?±sOeÀd?ō4[|RŒ?©–Ý…4ek?Ðó²µÖ«? :ƒJ×ýs?ØÊ´ÑzÓÓ?¦Ÿ.{o?ÖA™*¼tÃ?£÷y79?˜I®­y‹·?–?7—SÀ³?ìw55ìËñ?´­3À8ú#?¶3ê£|?±$êøµG›?Ÿ#ý¦MK?¤'—‹

?ä"õ&?ɘ/©Ìÿ?Õê¦UÙj.?ȓ‹ŸŸ²?«SZ<ä?š©W|D'?é ²ð'´{?±Uµù?¨]¦)Ü?¬Àzù?»ú8¼pDr?•ÛdJùº?ÝiùB÷v?²½^ų(?Ûè× ÷m?°¼û¸6‹PSR4FGL J1341.7-6216?ä¯Þ€˜ ?—F~ŽŠÀ8><ÓG:À:$ƒÁÁ@y'w¾'˜@»ÒÄ]''?¿®áÕGšž?½ðÍÝîÞ@'Dé>?ÿŒü?O?ïl™Pž~¿à¼ÃÕ­F¿æsY>	Ðä¿æ0šö奿蛪ëÑtÒ¿ãä"ŸR¹PSRPSRPSR J1341-6220?­òƒá8¤?¡kTl&?€Èٍyt'?Ÿ`s)b»?íë}qÅÀ?¢jÉ&ÃñÙ?³+œ_‹o¤?±8'À¶p?«>Ce8®?¡ä^Jme?ëæ¨=vX!?µI½Còç÷?³®-²7A­?¡¤:ñ
`ö?¬*>ìõ˜:?ŸÐs¥ˆ?ëǖZÛÿ×?§Q¨Fäª?²gnrP3Ý?ÆËPiÞ?¯ˆ¬=QK?‡•3cH"?뺇q½¡P?—û\ýèëÀ?¥í™r˜¨ø?—^öo?‡A2¸[?…'~àY?îD , ?/`$KÇ? yüìiz?Ÿí›õ™|?§hO¬ˆ6?¤]pÚ;\?íÛ6ijõ?«¤
	8ûÚ?®ú¡ÿAÛ?˜ÓÔÆè)?«Ê°B'(?¹4Xfh?ìSªáâÕð?¤§È7eÀ?—ÊP‡8?C+è×ër?²@IÇb?"—i¤?ìõ±¤lR?–"†¢U†ÃOTHER4FGL J1350.6-6224¿ÒI½/Ã4¿ÔæÒâÀ7ÞÓMŽFÀ:™c²VÿÁ@[Ë ýQ@EE\*£B?±$Dÿa?ÚyJn¹?@%sçÑ5Z?ýoçáüú?îlT‡@с¿ÑÕ­+ª~¿Ý,iÀc¿ãÛJ^H	Ú¿íã}zV¿ïÿw¿1cPSRPSR3FGL J1350.4-6224PSR J1350-6225??žiT¡>+?6G"¯t?ïh
–dŽ~?¦Ž9ÌÒ?'€3‡x?¦¼>pdR?}Žßu«±ª?…¦¿2_˜?èÑH¬á?¶áJ‹?ËÎfTó¢O?¶¼õÿ¡
|?xgmͺë?xŸ?ü:gÌ?ín±Â
Û?¤>!¦Rk†?³{z"§º?£D žäÀ?Y¤Pµ¯¹¾?BqžÌhó?蚢Â{ÿÅ?¤~vÓq?Íb,T
²û?¤y¡â¦?Pñ.?©DO?Dúz­öM?ï*'Ipë?"ÿÌP"À?™žªs³5_?"»ª50?sX
yÉÏ%?,"¡)UÆ?é–åøAð?ºZlº?É	§Ë­àE?º~™x?r»óǧï?bÒá6t?í䤬%?Ÿ¨xÇ¡p§?¯^6Âäàx?ž´ÉǞ¾?/°CO/ñ?p\"hÈ?éûÎ:"­O?¤í'.UïD?ÈÛt´?¤ëªðonlPSR4FGL J1356.9-6432¿Ûÿƒ£Ž"Àvò"º7À88É$¡ À:ÿ§Ÿì™ò@eÌ[7ß@?ÛÒú
x?±Ar'?Ö,?Ž‹Hž@çE™›@m¬¯Ëà?Ò àdõ"¿Ù¿v"2á¿ç>	…º¿"¿í*†Pçy ¿ìϦ›àœ¿ßŒ"2T;PSRPSR3FGL J1356.6-6428PSR J1357-6429?¥2¦–8X?¢ÎÖã>?è51»	?Åxö`ïÚ?ʺJ Ç?ÂëÀ‹~n?§*½é'ó?±32¶?ä'Téê·?Âå/ôS=Y?Ô(Uô?ÁVüŒ¿&Ø?ÈKysÚ?¯ãCºG—¢?â©=§½?µ3_½z«_?͐Ilc3?®ÏYeÄZ?¬qjJ^Ž?‰´Êޜ>K?äMZè?¥ÎÞ`M;«?Ó×)Žñ?¤º˜EETT?š'R{ÏØ?•_UksŠ?ç6qM—…?Ĥ
<U,?Ð}üQ—?ÃYBÖ-7Š?‡k½¿óÞ?—:¤Íœƒî?å ~.ró×?Ç»÷½fRo?Ó¶ŒæÐ%"?LJÖBí:?¿¥'¹?@?©Ž‹¯²Eô?ä~ú ´Z?¶¶¡ËUú?Î41NÆPv?²2XZɟþ?†E½Û_?m	jwñç?æԏÓ'"?­hC¥æè?Ѥ²k;|?¬¸B'ŸûPSR4FGL J1400.6-1432?îôÚ`;݄@FˆÚãæÄÆÀ9ɽaõ¾^À<Jã´oÞµ@"{±|9?þèm!kŠ"?»R´¾õ.ý?ÛRËêN½Ó@üC}-RI@zßæ¯÷Õ?¸µÓ9£¿¥TºÂ^3è¿ÙJT¢nªX¿çŠ×^÷\¿ïÿôa¼2¡¿áÎ"7blÝPSRPSR3FGL J1400.5-1437PSR J1400-1431?Í[g'£¼f?Åë[SôÚï?ç¤í¼ H¤?È)Mó;=? C†2K¼?r×ƒS?ÉüŸ|1ª?Ájï«&½b?æ†2½¨¨¼?ÃfIž4?·Ö^Òx|K?­<=»$îG?Ɔl­Ê o?±Þ¿ô!O†?çPGõ_?´2T\•Û‰?¸pæý7":?¡ýØ/òÛ?Ý¢G¡‡Ø?­«ü%'b?Ûm/@½èâ?®Öë<W'?»ÂÅނ=?"sB7 Û?¼¦pd
"?¹Ô68 Wä?ëL¾, {?À&Î 		ê?¡ç<w›>?¡'e×gˆå?³œÓÀôáÆ?´Î±¤?ê·oV`E ?¿Ñó¹[è?¶§±ŠQ':?³§jwùþã?±¯Pe‹.¤?£^A$ž¬?êÐÄÏ0?¬<ɍfÖ/?·Ê‰"¬f÷?¢QU'çµ?ÏkàK¸BÛ?ª>]9À5Ó?✠|·¶?²Ì÷ƒÉh?Æ!Áhâå?£'iË$õæMIXED4FGL J1402.7+1306¿ÅŒÖ+ŠK@Q
Ž`€sXÀ;/´yï°'À=Ag2>@­@Ù0«ï\š@¸/ÿ¢/?Ïn"3¤?ïÿÓT¦J'@j†!퐒@¬ô•=¿¿ïÿÿ>¹ú?ïÿú÷''ý?wäò"䣿çVØ߬޿ïÿüÚ±'Þ?ïÿh@S§PSRpsr3FGL J1403.1+1304PSR J1402+13?Â`êf™E?ÇI9˜¹Ë?ê>'"M»†?Èäæê/^<?¢–£ù~Š?­Àn8˜?Ñщg×Æ?ÐKêÿè­ÿ?äxO]	%?ÑYÒë[?´÷_w:ÈI?±%ôïOh?ÜFº–‹¿‰?´âèg{òç?ÜX''[ž?´h0bS?½'Ï_›"f?§˜á4´*?âcŸÑä[+?µÔ*>`ò?Ù±qÕ¸â=?´Ù‰«‡O7?˜tèižDÈ?‰Jß(¼Y?¿2Ù ^ž‹?Â*¹(Ív?êÕ_*æf/?ÄþÀã"z?¤DZpþ?²VIÁµ¯‰?àç
7B"?Êyý¥Px?èFv
è?Î4dÙü?¸[*æ6?¶A­f®t?×óÌÞóôb?²ÇÜàܝQ?ങöÇÙ.?´rAAz?º‹üÍñe?¦v
×ÌŸ?Ì'Y؅à?µ,.ìƒtµ?皣è¬k?·ØCP÷9?¦U2m'½Ê?˜7bãg'ˆMIXED4FGL J1411.5-6133¿Ð­™\÷Ž¿Ãƒ'ÓÀ8Žìø¼>àÀ:ZD4"@êýsޟ@1µ"±«?ʔk¿ù?×¥l`¦]ø@"Åyò4e?ô³[,°ã?é­Mî\ê¿ëPƒÀê@{¿å˜fÙS¿ç…NSJ)ð¿ïÿÑ;ÇVk¿åwÜ{~PSRPSR3FGL J1409.7-6132PSR J1410-6132?ÊÑXLÈ/¯?ȲtáKe?Áåė–"?Âè5±Æ>Ç?äÒ8ÆèS³?ÌÁ7i	7? F·Ê\/?ªU¡Ô
¤?ÃBþÏ ´
?º_óI}f?ê%kàßåj?º¥v8Û-?Â=«¥=oU?¬U=ŽÊÁV?Ãy¹™-&î?ªw'8ËOT?æ'&°eZo?±Øïtž`É?tqÀ¨p?URŸíÃ'ã?Æê¼€Fj?¢ùDqkt?êm^}8æ?£h!ˆa?§¯ÄAL¡O?±¦W ®ih?»'Óºþ?½á*Â?ë!>È#?Á£gùŽvÑ?'"ë³+‹Ö?›'">{?™U¯'‡à?¿+¬Mº?êÍ6*?¿½«OW4?¶Öiç¹Ýé?¢¬·[¦Ž?ÃÔ¿ÑLõb?­öÇIº?è0ÎÞÂ:?±§¸W_-?N7÷·?<…rzÊ?̀|~ή?®nsžRÿ?èØYÒsÀ?®i@0RËWOTHER4FGL J1413.5-6205¿ÊÍÝΧÃS¿çx;»²À6hz™#RÀ:lÞO¬@tðo"7…@ªWÂ^´Á?—ZâàƐ?Ö:[4GZ@9cœ¥½"K?õø‹Âku?ïêF$§5¿Ä:òÚ¨'–¿ÞK9º5ñ¿ã|¯ŒwG¿ëқ
7 (¿îÑ݉¦PSRPSR3FGL J1413.4-6205PSR J1413-6205?&B¥€µ_?'‰y&,ë¹?îm^¹Z?­‰M?¯Òçm1è£?¬ö¬ˆùR+?sל[yf?"næ±0)`?ìØ3™ú+o?²=÷ú{p_?¸énâïv?²–úu*
?'ÜA™YV(?†v؈ô"?ìè­TÈõ?¦6ø«"û?¶_
*Û¬×?¤®ŽÉ1ç>©·
;j>©¦'"o?îâlK$8?S[xŸïŒ?¡Ù!˜üǯ?S;k"ì
?6fb$Ɇ?4ê2iíg²?î
žs?Š&?¬(D7'ž?®ùLš}é<?¬yç8
,?hϏ<hS?zD"þÒºj?írMzå¬ö?³tÁ.Ȑ?³§®uÞN?³BIýTH?u´ƒEÀ?{R#ðìX?í²EÒÖ§?¢^é4*ŒÃ?±ÖÍf+¬?¡Ó P—òû>€Ï&¡É>…Ê•æ†PÒ?îµçZŸ?"ö#Sl£?¤¯½…L©©?"ö [©ÄÁPSR4FGL J1417.6-4403?ŽWcŽü¤Ú@0!æW¸MºÀ9~VG4À;õÐÕp	}@õèä°nG@wCõ"V?·Â<Pg?ÐÒpû•¸@%/ ×{|?üy/ï[íç?ìÃãNïQ\¿ÛÉ#…–,¿áíp¡'Øa¿â"Ànš'¿îà@$Ï¿ïýØ]y­ÁPSRpsr3FGL J1417.5-4402PSR J1417-4402?Ü"ð,DÎÞ?ÁŸ¨ ø¼?×b-üì?Ã\Œ»î5Ü?Ʌ[Mrhl?¸sF–?Â
ã (òñ?¼Ôȼc?ç©«܋m?ÁŽD¾Zï?¾–àèɾ·?¶€Ô½yK/?ـ«/²äÞ?µcŒ¸ÒÈN?ڞÁR+' ?¶õU"øn?ÇÁ&þhó?«ooO"}?Úº€ïԎ¸?¢ý\£Ï:?ÖÆáwQ?¥f̯ôä?Ìý;28¿î?ž¹'|Q±º?Ã'´ÿŒn?±µ0Ế¯?âd'X=¿å?ÜY"Â2ü?Ñ£Ïú9ÿ?À$.!jM?±É¯Qø×S?°"p8£ê¾?鞮Í5?Àڏ(ãŠ:?À m!°BÂ?ºÑ9zíSw?È$ê)Ä?°ª/)?ãÀBY…œ%?·EÛiy•?ÈÚÀu¦?­
o š?ÉZœP$§÷? U•7ÿ§?ßDD
Ý?±<¥œK"?ÔQm"ßÎæ?¬Ø˜ PMIXED4FGL J1418.7-6057?å¢#tƒ?À½ªÛ`cmÀ5÷'7ËHhÀ8¾èyÑ@ 
'e¾—@Ât֐›?uHऽ\?Ö]þÛß@6åÖZHŒ?÷¥óýhK?ÒJ»¿à€£ßÓ¿ÒRHù꽿åB
 À>õ¿í]+TB¿ïÿý`éNäPSRPSR3FGL J1418.6-6058PSR J1418-6058?…Öu†Ù'G?¥²™©`–V?谂×`NŸ?̆²	ð«?ËàK$
?Ë,G72W|?k"7j{z?yWÉØ	B?êLד>$˜?Áa©2"Ñ?Æ^TÔÑ:?ÁQÃCX'´?–£ãÍÙã?"A`&ï©?é)
.ß?²)'­µS‹?șvÇe7p?±ZPݬݳ> É<°Zì>žÎ©YñZÃ?éJ?¶›ªb?³$Œ…T«8?ÊÖüóÓnI?³$Š$Më…?±h'@³
.?͑äAf/g?æ™@ P\?ÑÍßEd'?Ìæ´à	÷?ÌSžuÿê?g¸›[c(?w8/ƒ?ë«t™@>›?ÁZ¹·Nê?ÀóK.Ûh?ÁMô2J¿?ˆïþÜè™t?Šxp\¼÷ö?êOí
_-?´®E)(8?Å1KÝ#12?³5®XZ™…>i͛Ч¾>qԔ"º›?ê'n9™~Â?µî¼Ì'£?ŶF²…½ˆ?µî¼'L`YPSR4FGL J1420.0-6048?éÜט$F?͈y¡+´9À6­ûmÊÀ8·#24/²@ )Ve'V@üÉï£?³:à?Šj?Ô
›p3o@'^Ÿð˯–@`C¢?Ý?ï©¡ue¿æýôµÖ¿áSS.{=Ž¿æú˜'Bdÿ¿ìC[ªÌ¿ïÿöùŠpPSRPSR3FGL J1420.0-6048PSR J1420-6048?™Òvþ毵?´Ó]¿á?âôÁ+gý?еMæNg?ØyVÖAì?ÐcFÛJ'Ê?‹müþZô?Ÿ©d9à?á.8©ƒ‹T?ÍFŽÔ2‹‡?Üǃ=Gð@?ÌÍ냤ÃL?«€½?;)L? dxž£ùØ?âx;Ûãù?¸æ"\×®?ןp¢nCC?¸(ùkà?1«§ÂZù?!ªcžnH?¾2âëȤ?£ƒ¦KÛU?ì7n?½t?£…êz²£¬?©Èé›îG?Ȁ vyü?ݳ䰻–'?ÏscYÁ'\?ßþƧf?ÏC؇kÓ?ƒi'eVê?ýi·N—Z?âídͽ–,?ÎÞ$ù^¦)?ىéØ÷'"?Î~Sð9†? î½d.eµ?™îê8*"?âÂd¿zÝI?»¹œ7Ðô?Ø]^Ô»rv?ºwÞ³Õ)?	-ex4û´?ÿhB|âá?Äßþì`¿?®'^ǦÓ?êǛ_{]?®"Ãý×lõMIXED4FGL J1422.5-6137?éÜùÞ'èý¿äº'J9À7¡77¤²À;
Pø@@ €iڏ-/@Þý'¬?¦¤§tù|?áØì`@2£ôDàÚ¡@l
%É?ë´‹g\?ïӍæÝð¿ÉdxÞ°¿ÚS'Yáæ¿ë‹%nú¿ïÿCý…Ò<PSRPSR3FGL J1422.4-6137PSR J1422-6138?'î+¥Z‰Ÿ?'bRI«É?ïÓv^v?ry'ˆ_?u…_•±Áz?rí2Û?xØ^©AI?Œ¬Sà›Äi?ë_•ºšxÅ?³Î¦`!^è?Áºæ ìðÀ?³aLªùIu?¤þט_Þ?ž¡·ú)h?ëmŽEÓsÛ?®wŠªWEÑ?º&}˜1:?©F
ýÚæà?Zpg>ü>æpžRÞ?ï‡]"'6G?~
0½íù?Ž™öþÒî?~äf'™z?2ÍÕíƒî?*À@v-ž?ïÓ¡s"ܧ?r7CÎeÀ?uYj¦½?q¥ôéþq?oOBÉ®?zÐK¯›V?ìYpiýþ&?³¤
ü¯øÝ?¼8ƒÃÞ*‡?³z=¯â&?"ö~C%9?"FNùV¬?ìPHŽ¨éˆ?®¹Ù§'ï?¸@6lÑt?«í>(Ñý±>Ֆ•c}X>Õyñ3,?A$ô'?€G¨¥ðþÒ?ˆ–<ï~æV?€GÆB]2PSR4FGL J1429.9-5911?Üä%¸«?ôÜfŒ
ÀÀ6äh8éÀ:'u>p~@£3K[ô@Þ~pHg?˜Öoý'»ö?Ò¦¸¦¥@2PwxÝap@hš6Íq?ÎÐ
YË"¿ØÞ$þÜ¿äOC¿ç£ˆXÿ¿í½ªOÊB¯¿ì¯ÑêBÿYPSRPSR3FGL J1429.8-5910PSR J1429-5911?RrÂ@~?Te]s'?ïW`«?"éÓ50B?"öãòdS??"$''}^?tïDPNèj?'	&£ç~?êX‰Y©?µÔêŽq?Ç7#¶F+;?µPH=)­Ù?¢ê*;ú?žLæö_;?ìì
ÄÜ
?§VP¤Ë5z?´ªæIý³?¥~¶K
}? 4	ñãVM?K"£UÑ?îD5j‰Ð? &`ëû?«®X™ç?X›¨Z?UªÅӖº÷?P£cB'Á]?ï$¢ªËY?–·,Ô(Ê?šþJ¶A!?•|e•ÖÍt?lÙuå"ñª?w6ó‰0Š?êÔ9ˆŠ~?¼Ä¸°yô§?Ä;¶
NÉ£?¼°X´'?}»·O±Ê?}]«Z¢êü?íãÀM|Nt?¡<Øǃ—?®µD¯'? OÞý‹bs>ó¤;ú®]>ñµy'Ì?îZP›£ßï?•Ú^8x)?ªX¾‰ý•?•Ùl©‡´{PSR4FGL J1431.4-4711?íbS×:'@(§¥	9d¦À9È9¼º0À;ã¥{O+·@x1ü@òR}{Uâ?Àª}—…m=?Ê®ÿ…Ö@%¼Cè@³æ¥;
¿ÙãEó¿Ý)´.pV¿éI-``gõ¿çH~ôÒ¥T¿êˆOúꊿÁë;¢ÃcíPSRPSRPSR J1431-4715?îx>°iêª?›)ñ½ˆf_?‰Û¦7r?€F•b>?¢ž‹^<?—Û›Ú'=?îcDý{Z?§Á,Xï?ŒpA™móÐ?'Ÿ¶¯=?¢¯­ÞPc?£¡<Ï^å?ìËu6Û ?¡Å!*Ÿ?ŸŠ'úúî¯?"»¹Bñ*?±Á±ËˆŒÓ?šU['"?íÁJ³é?…pÏ4«å>?—Foò(+?sΈ&;;]?¨H&ÍX¿³?ÏQ­`ç?ëÞ9NÞ½ï?°øJ¸º·?¦ay7g?ž0nž€Ò?¶
¨×qÙ?«C;ù\K%?ë¢÷+E((?¿'EçY¯¹?¤A¬¼™ËY?®)N•Ö?¸ÇpIA§?¶ÃTœóñ?è!sf:WÑ?°WË@v5é?µð@‰t?£á>­fŠa?āñÇ­ÿ?¨-¿bÎMÎ?éÉ<æKŠ(?¡17•Ï|Ù?°·@MÁâ‹?'›¶¦‹l?Àl>9?™¤Ý\¡rAGN4FGL J1440.2-5505¿å¿ºž)ª@%4¢žûÙÀ9ì"ì"qÀ;b–ãܳË@´"gÑK@óìÌG?àåîqbBë?Üdrûö*@?,0	³@"K>—ÀQ?ïdG!ý€Ê¿çK;gµÿ¿êLL¿vM¿í¹Ò9?Ö¹õ͔ô¿ïÿþó…õPSRpsrPSR J1439-5501?étw,Èá?Â[ÌË[nÍ? 	ºáu?¨À_-u?Æ+µ<¯« ?À+èP¶Ñ¹?å|ÐÚDý?ÈË¢ô>ßA?—Ä£NoW?¢Àwž¯ôs?Ӌ'(û»'?ÆÈ~~¶x?æf½3x?±OßôïA?±@‹‰'í? ùppŠ¿}?ÎòXÄߏê?®²U_¢?êßX¬?©Wq#þ!?kOÄz+A?a—å§ËžÂ?Ä` é(?©'Š]'€›?ãf¸ú:¡Å?ÇØÖ¹Iž?Ãju¬Kð;?Ãñữ?Îú¦jɈ±?ûä‹õ?Ý‹iøc¡?ËuOÒ?£ÎÔú°Å?³½þ¾Y?à8Ù]Ý^s?Èû8?Þú ¤Ý'ã?´uzýH×?Â彩Ä4"?°¿Â	Ó¨?ד†@T?³ov™X?á3\\æú?¾H%ç"ìó?{Xª÷?€ïsò"RJ?Ý,Þࠔ5?¾i!"œMIXED4FGL J1446.6-4701¿Þ%ü­©á@&×W÷7ÚbÀ9¶Ë¢*aÓÀ< #‹öC@úÚý8?ÿq'Ñ8?º'pÉÂ?ۏç¿€Ë@L÷‡‹z@™·
ó³–?ï÷ €=¨¿ãœÀ€
V€¿Ú¢J"
¿å1&s1P¿íˆ}ˆkI¿ïæ¡à×PSRPSR3FGL J1446.6-4701PSR J1446-4701?ŸKöìt?J$l±?íøÀfô?«>^ãÏÃ? òS"ª? [ŠÇÙ?²âã6Ÿ
?²òBEÀk¥?è†áNË%i?ÁԂýåR?Äs	*(Ñ
?¾ŒŽ·¾H?²–§‰·È[?¡‡ú× <?èÄ­=)E
?°ö:‹­wç?á÷GZîŸ?«W¢Õâ³?ÐÕÑyme?¡ØæâQã/?ޗÇLZK¦?¥¹—,U>8?Вg¯f6? ÚúbZb?ŽÖZ¨7?‡èEõ<ö?îUBSPxØ?£Ô³`•'?¢öXò–}3?ŸaªÜ¾Ü?¡²uGO«×?¥|™
¬?éßêYá®í?ÁótŸ9A?ĹG@T?ÀbÍ&8ú?¥<°5l']?™¡V_.Ïü?êdURþæ·?®\bÚÕHþ?Á~¦à:N?ª0¼YŽÇ?·Ê˜o¯¹?•
Í8j?âºg[3û?¬¬7´k:?Ԙ‹.>N<?¨ÐjdmðPSR4FGL J1459.5-6053¿ê­q™0¤I¿üªØ>À6ÎÿÄpݹÀ:p™ÆC@›h,**@ՙÅ8ƒÕ?–ÝB÷݂ä?ÑsUAûÍì@3fÖE"@«"Ï€0g?ïÇ€\±²¿Ü ïCš3¿ä_Eà´á¿ç—×øyùÁ¿îVÁ"¸Ó¿ðPSRPSR3FGL J1459.4-6053PSR J1459-6053?]™…Ðù}?rc&-wŧ?ï
»ëå'? Ð~÷Ə`?œnê)» Ž? #¯È³w?|&¾ˆÎߎ?‡Ì'áE¼?ë-UýÒB?³r§è©Ü?ÂirD…–?³sa?¬›+Øà|8?¡f³hg?è§ÓQ(ð?±‡êüý¼?Æ9çÄí&×?®™t[ï?G49ÍÌ?‹r¸s¢¢?î§^?ó­Y?‹àŸ¡ý?¥ƒJ24Lç?‹*Ö1?ŸC+ue?øoa{‰Ó?îTºíQR?Ãn"B€?Ÿ²=)-½?›¾u¼²²Ì?røʵ{Œ?~Çj›Rú?ëï'¤£|¶?¸¬aëk?¿W6-õ—Ø?¸ƒTœ…r?¡ÆfP*¶?˜™iänUÓ?éh"âFB?´OçÑ s²?ÅíïÖ«â‹?²yYŒëÃ>àr,\…Zá>à)–©`Ð?$Cðß?"½íÆHw‰?¥%æšXzM?"½r‡tžPSR4FGL J1509.4-5850?ì"Ó±~¤¿ã¶¡²lÏ6À6áÐË_ƒÀ:,…'¤Ø'@MÒ±=OA@$³"כ]?žœÁ}t† ?Ø¿Ì^<÷,@3¿â`²È?@¸l"}Ðæ?îrjJ÷u?ёÖ¤¿ÝìWڎ¿ä‰Øá®a¿íW®rn²e¿ïÿÑ ïcÑPSRPSR3FGL J1509.4-5850PSR J1509-5850?O1Hù?_ÝÅ&h-?ì¦NÁ·£x?Àl Svcx?ºŽO'Ôf?À=còé†?}U}D€5æ?Œ›v¹PáG?ë/Œ=6?²G»kh"C?ÂW#ÑÖ?²Isº­~?‡y·B‰Ù?Š<3j™.˜?쉟õíò%?©Wl'>JW?¸ÃΛ_ë™?§œ×¦?{]?uô¸¯Ö'?
žr_S?í'…"L†?š«¹åf)?¶¾uÿ³o?š§ƒR³?QQÀÇBå§?P@ÖCQÃß?젎àzv
?¹?É¿L?º¶Aù}7—?¹ºÒfy8?n¤4뀪R?{¨ã|OP‡?ì 3CEÇW?·	§½|Ù?¾	D;2û?·÷ˆËö?{X™Åž:?¦šÇ3¶?íˆsxêð?¦/KÆÆw?µ^2ÆÖ݀?¥A	¿Ú;™>ï¥:r,Î>ðvi¥êE#?íD8Ç¥N6? )Û~gûA?µÝ<˜¢þ¼? )l…ÆEMPSR4FGL J1513.4-2549?ìïVv@:ö—Oß;À9±WVO˜À<DC;¾òï@ç笳@ÃÝ:ZM?¶ÿ‡_/es?۝}ÿµ,@³Ñà2_@6ˆ*?î˜?ËG¿É£u{S¿àBuüŸ|¿èÊXÿ°J¿êþÈs¡¸¿ïûý<aOPSRPSR3FGL J1513.4-2549PSR J1513-2550?ºA|eðä?³¯\	ÒM?ëÐ¥ú¥øø?¸:÷#—È?Ò:¾Ð‡X?™ÝL>Š?¶^Ÿž*?³Úh·f˜—?êöl6›-Õ?º!ÆTË?²E?º=³?ª8ä½£Fé?Ç	Úzƀê?­•g5_?揌õhIJ?±kN¾»"?½oã_,؞?¤ñ.ð®?ÎmJõá\ì?¢—W¨'ß?åj·\´G+?¥ì½Z£k~?·Ï¯,ã>Ò?™ZJñBì?£Iq?Äþ?Ÿàʓ^,‹?î†bVý?§ré;úI`?–ÜQ<B,t?':ë6ºê1?¢<:÷Uj?¦X'Ê9Î?ìô VjM"?´BÚç÷Þd?®ª¾`÷‡N?®}Ƶs¤C?·Ë¢Ûçã?§´<¼¢˜?麄ñ@õi?¯7Â)©ÉG?º`5›~‡V?¤î¸í¸Mæ?±'úÆ°(&?'Ë™ ¬\?êtâ(ÒW?¥åÛ¦)V?ºÕóùÈ?¡ê/ŒÔrPSR4FGL J1514.3-4946?·™·@ôfð@<½±¦×À7ëýŽ5¸IÀ;t]ýâŽ@"ÜÅ×?ý;v­‡?¡UÑÿͼG?֖!_K?@1,M‡rO©?ûiùée‰È¿ßNa6ü–¿É‹¶ÂtYC¿Öå+ž{޿ߜjÄÄ낿ìë€K꺿ìÙä!þ£PSRPSR3FGL J1514.2-4947PSR J1514-4946?gßs7¯?j›ÑšKw ?íÎaBÌ>™?³$׸;¯Ô?°Ðï«?²ˆSƒI#?‹;¨¿Õ­?¥MÊÁ¸OE?ì•
°íž)?¹‡2‹+Z?·å«
 †?·ÞIðæ'Ø?"]zˆ»?'·Z.PžŸ?ì`Zy¯T¨?§PgÃÕú•?·å͏?x'?¥õªå¼ö?Qz¯fT?Cà¥îgCÐ?íô™njZ¬?"	ê*#ì¤?°L.I
?'ßÅúöK?k¯"‹¨Ç?g[&"pƦ?î=v$
j;?§ŠŒ
ÿlé?ªm«•tºË?¦{Míãa©?'ªÿþi†8?•wº)a?ìÃiC1û?À˜O'RÑ?¹,"¶f6ž?¿ø­©ì?‡ozö¼?‰Qkg +?íBÖ;¶d?¤Ý‡ö}!?²û^Á½‹M?£Q¥ñè?34͛™?+±Tk`?í¦Ù?s'?šíoØË ·?²¶0æ¿?šßVlg?&PSR4FGL J1521.9-5735¿—L¶^s¿ÚZyMBÔÀ7N#'¬?À:ƒùd@ŸĈ/º@ûbó?£Ó›s
"¼?ÛzA—b@/I¯:ÎÄ?ú0«?ïҟà·ö¿Ñnñ$oöÞ¿â'†ø­%¿èç/N¢¿íázn['n¿ïûÓ {‹PSRPSR3FGL J1521.9-5736PSR J1522-5735?CÍΝ@Ñ·?@ªpQÁaC?ïJ}n&Š?˜ÅAîn?–î6vV?˜páŠ63Ë?¤q%¸?4/üTÌK?ë3Žf¤h™?±Šº6OÑ?Â4¢ÝBÄS?±@†3q'µ?… ¢/;î?…ô]2Ö¯?íg*9B?¥LýÆÀ?´x²h¼dÇ?£ïÿl\I­?xód ô?	¡ö2­EÍ?î7KϦ
?Žô\^ê'?¬'Ëeg»?Žð£×æ$o?SŠ‹
,?Tš	BD™?ïZ…ÌL
?Ÿõi¼ÌC?›c–­tû|?žèBÙuP?p'7Þ)Ë?zƒJ£wJ?ì4®ï}b?´Xl	µØ·?¾lâcYc?´45÷½ÿ?w,{'Þd?wü'rê¨?íï!°vLZ?¡2Úc\r|?®(U‹W? ÏàÏúXë>êéDºŠ¤
>ã©sÛ'ÿR?îúŒVBµ?JŸZ®	?§Þ¨§µƒ^?IÏƖÅPSR4FGL J1528.4-5838¿ÃÓUÊYLo¿ü\¼™yÀ8Î.«6$À;›mµæz@ ¼Êv0^@(éÛÑLŽ?¸Ö—Péý_?äi›Ô×]@#»úëÄ?ÿ#á?¿të…tž?ïIšé$ò(¿Ômc°©€—¿äÀ|A™þC¿í蜁U€¿ïúÖàÌÞëPSRPSR3FGL J1528.3-5836PSR J1528-5838?UôôF€ó?WÀmå½0?ïrÐùÅ?ž‹ ¾™0Ó?œ?¶§±P?´LÚ@9?‡>W#‰dF?'öس»?éN½Â?· ðÚUóé?ÉT
i÷{³?¶ÂzoèN?Œ,J†—üd?"mR­è¬?ìÊÿ;E6§?¤½Ê'nØ?¶"|ÖM%¹?£½'œ¡?w³"¥sÑ?\¤Î©5`ç?íö¸¿µÉ6?æ7\+²³?­ž£fd?"1ğáð?Zæp¢-«?Uaá¡ç
,?ï,á|~£?•nÙ®?˜µo¿Ô·j?"TGˆˆWÛ?x¼…Ò8±?ƒ=Aq"ä?ê¬vkNv?º´™­Ä&"?ĈF.§L$?º«,î9r×?ˆƒ˜ä3¾?ƒ"( êe?ì‹FlöÎS?¨~A¤e$?¸•Y"­ð?§=¤ŠÀ61?RWmØQ6"?>.5¶¾¨?î|ˆŸÿÃ?03ê¸ý?§«œ
'›?wÅÚ ePSR4FGL J1531.5-5612¿îw…ï²nÁ¿6pÇ¡À]ÁÀ8žo¿«À:‹Á#K^£@")K'ñŒ@E\{+‰?À܃ä{•"?âßøãú@×P +"@½(ûL¿ïûü€¿?ïÿþBe«+¿â@`xÜ¿éÚÔ,<ží¿í…H©¼ýL¿ïÿþBe«+PSRPSRPSR J1531-5610?›JE¶}?¹±—
S?îaë
pá?»騶Ô#?˜²Qú³4×?£&™uF?˜áËÁÇщ?¢â$	æ?ޓ.\k?ÃáJhf
?ßÞ´çäç\?Æ]îƒçè?µWJÿ'žó?¤ä·U:pÉ?ä8½?;)?µÎf~.ò?Ò:+ŀ¨1?²ÜØà5È)?'Á!¹\YR?r+j²ëk?ß½4¥?«èºïù¤Q?ßÏ0Un'¦?« ;4¹?ŠX("¥—\?¨9–S$P?î¼Þ¡Ð8¬?­&a
øE?›8ƒVÍ? ,óßþ[O?Åõö+?†¯wòíØ<?áƶ6¢[?ÉE?ÁPª?Ûê5cB8?ÈæúˆÐQD?¢ÒUÔ?—˜1®†9?çÀ)i
"D?µõ§oA?ÌJºxâ>ú?³åÛæ–¨?m'ô5ÏID?U‹ö9øà)?â®\‹B?³f_
4Nš?ÚhBbòØ?³LêµÞ!HMIXED4FGL J1536.4-4948?¸ÅN¯3¶p@%‡CUÀ&À7D¾'wfiÀ;i
	Ó¾@4è-?þXAZ=c8?™t-EÕĐ?Ï¥}'þ®@48ð"aùð@+SÔhx?ïø$B`M¿ÎÒ&þÇp¿ÝÔÜeÇ¿ààÁKdW¿ê7Pþ¿ï-¨§b°PSRPSR3FGL J1536.3-4949PSR J1536-49?‹ò¬ìmã?"nröØê?êkŠß[^?È@ŒSA5?Ē©²¸ÆÓ?ƨàÿ‰¸{?›«™ÒŠ¸?ºs8ØtÜÝ?ê»ÝXá²?Ä%0§
¾?Á›)
T0ž?Àj–ºÖ?Å´+¿"ð?«ÜºküFp?âÀåIµ—?³îÇ@ÃU?ÏH?Il¶?°çÊü›¥?9TC¸¦*?2`#î5É?î@yê-'?"
—Ü˵…?«ÅÇg5­Ý?'õ<¸ç¾?ƒð•"8ò?…Páú{?ëÒÔHõšÕ?À	Ë6Zì?¾ëKm™z?¾a­šžf?"a¾S:Ï?Ÿ›Gˆn'Ê?êí_ó5?Çí°G0G?ÍxùA?Ç3þ—©Ý?¼…lh€i?ª
ӕ}?䆊A"Q?¸¶ÉÎ1ö?Ï¥ Å®‡?³¬IÊûò?F'HTM^?6
RhÔ?í¼Ùa}ö? ä€díª?²cköxa? 
e¬Ô 0PSR4FGL J1543.6-5148?×5±¹\=Õ@ù#zX‹²À8À/#ÙùÜÀ;3òuÓÂ@wP»¯C$@C‹«`k?¸ÓfC«Ñ?ÕY:Ë@7Tm?ž|@
jØf¿ãuIX8¦?ï³±=$M½¿ã˜Æ5¿åÃG
H¾¿ïP²4›@¿ïþ)ÉßPSRPSR3FGL J1542.9-5141PSR J1543-5149?§]ÒÖŸ.?¦ÇŽƒÍ?ìüë‹ÝKÿ?²\؇»×¤?¨Ótlõ‡è?£wY9îhr?¬cç±Ú¢?¶ֆ|3í?äaì¦~Pà?ǒ)K0ˆ'?Ó¯©¼ã†ß?ÅÉ$	'N¬?¼­Z§Ò}¢?§ä\™/§¾?åöéÒ}L?´{4'›?ÉÍ«_ûÏU?°îuQr?º$@Ͷ½Ó?'›™Ëƒü˜?äoþ¯aÇ?§ìy݈4?Ñ8Ï3Œþ?£ïþ(…n?'æ«)ÀÂ?‹øvûˆAÆ?î6žg6©?¢¥X"º¾u?£&9‹Î?œZÅ}µþÎ?'ºbÓ9…?ž\IÝï?æ)P0gã?Ê/
D& ~?ҁ¹Ð¾q?ɎóÉ÷ìq?¢Œ Fҏ?–…ÉzD?èð4µ¶¨?´|\³§eI?ǜ,?'ÖÌ?²'ÃÒÞ?›>ïx+?}䟀|$Þ?çkÁ0PC©?­ß@ó´Cô?Îðs^á%¹?«ì›¨eÛPSR4FGL J1544.0+4939¿é:6ûMa@Izd×ñÀ:ii˜JAÀ<»´Ci@V3Á£xë@üÂ]Þ?¸Œk2ÓçÉ?ÉBÔ+'@ï|i+?ø
ˆ?ü?ë08AíH¿Ë|ÊÌ¿á"lhÞæ«¿ã_j^B«v¿èÈX>/'¿ïY§ÜR{ÎPSRPSR3FGL J1544.0+4938PSR J1544+4937?î";Ý&?·
Q"¦V?'IK'>uJ?—
r˜ô&?¦')DÚÀú?²`Xð²J?è;*ë]~?Ã>ŒkwÐ?ÃÚf©QÀ?¿åS\a?¶qÜ{Sxò?¬	¶Æ§Îù?íœÊ'¦? ~ýÛêJW?¡Wϋù/ó?–cÂׇd.?¤Û†ëZ?•Bi7û9µ?éf–'ûã?žP²Š}i?ÃL@ Y&?œLܖ]=â?­•nB§;?…s®»yD8?ê~Ã[‰é?»—wbYˆÕ?±£•[?°%敟Ô?ºlIÕ6'Ú?°º›¡Ê?áÉ&4ПÉ?Éð½Sg?ѝ˜$W*è?Ç÷Ýÿq‡#?Å 6ä+?¹™›XFÏ.?ë"û7ÌӋ?©µáfÌb¦?±›þú?£t ü3sž?²H	¥}¬?žài`›y?â@}Öðg1?¬ÏŸvø‡?Ӗ´³Œ›?®*OÙS"?¿¡>zJZ'?›ˆ{÷ã AGN4FGL J1553.1+5438¿æ§ËÉËJ@G•ˆ†aÀ:—ù_ÒÎoÀ<Ìò8— C@¼<Vžó?ÿhfx?¾í‡¾‹ý‹?Òó†ŸìÄå@ïÒ¦*¡"?úݹv®³?ハŸ€¹N¿ÑMÓؿރ{Óö¿àïgAÒé¿îgÝÿú÷ƒ¿ïòO]‹KxPSRPSR3FGL J1553.1+5437PSR J1552+5437?æpeˆ~O?À¸ÌF·kß?ÆcûÒô¯?¹ùR"å¶?¿´ÜŠ¯`?³½H$'?Ü÷òW`f?ÊZ];HÖ?ÛÊ™÷.í?ÈÎKrD@!?¼÷Ô@E«?°¦"	'î?⁩ê/ðD?³å
½:Œ?Ñm¿v"?°§¼`h²?ÃÇ#y›'/?¨ƒ¨«*FÃ?å^TDX}"?¦Kg¢§j?ÐgÎ)‡ý?¦5Ë¿¶­´?³n%:Éo?Œ'3
>Sj?ޗ¢Žù?IJ7£
?ÖƒÏËQ?ċ]Ž?ƦÅ£Kl?¸wxÈÃÈ?ÑÝk¢Þ?ÅÏ­80Š?⁘	š?Ê>[ÓýÝ?Ã͌ÖUY?¶µRù_\?ܼ›wüL(?·¹pØzíì?×èÍçÝ?¶1º]ð‡M?ÈbŸ@'Ys?­£eè2?Ú9¾ñ›?°I(ƒzõõ?ÜÏK&ïØë?²Ì(õp½?Â\ö6cÐp?Ÿl9[¼¹MIXED4FGL J1555.7-2908?݃®	W@2€‰ÁµA–À9°^©Ã)À<y)·‰o@¾€+ßVè@x¶Ë?ºˆá~<ò?Ï)U–µd@
\¶â¼y@X=®·8?Õ;Ä|FM¿Ý¢ˆá:˜¿é	ß|Ò¹¿é!YKË°m¿èÒUºc¿ïÿ¨âaßnPSRPSRPSR J1555-2908?íO¶öʑ?ª°Ä±
?¦eÁݧÝÌ? ÷qƒ?¤žÜQ3«&?œ^ï~ê?ç">þî]?ā‰;—I¢?ÆxfÕ2]1?¿kèGÛ?¶í:^–Ps?±¢eΙ‰1?ë+¢þr6S?§'<laÎ?±—Üܓ? 'Tí=Ê?µþ2P?ŸtºtØ"?êúŸ Ÿ»?"Àw}ÔM?»Ü°7ÉMš?'CďŒ\?´zÍyæŽ?†¨"øäDŽ?ç\ÈNҏÉ?Àéú²?Äóù#9bo?ºô歄Ä1?»1ËBø¼Ù?­Ñjl4¥‡?ྗ¶¦«â?Êôƒ?Ô§ó²ra$?ÇqEZ°®<?õ¹À€Ž0?¶ZN¯ÂN9?æ'lyÙho?²©­Ø:Ë?šçà­?¬ßçöb·?Ã[f7íW1?¨êKôíu?âÈÍÊà?¦M9©ûÙ®?Ðâ¤ìDG"?§Ìí WÍí?Åò£@EY?›bWa[|¸AGN4FGL J1600.9-3054?µZ0LHäè@0o‡z³$…À9¡çÒ␃À<lU\Rç.@!›_íP{?ÿd1m`U«?´£×àýz?ßü©ß7©@"ëØYÈÉ2@Ëuå	"Ž?ï´~÷¬Ê¿´FÕQ€¦.¿ÁÚâ9Eœ¿ÝUÈbÿ¿í]v¾"e¿æßnàˆktPSRPSR3FGL J1600.8-3053PSR J1600-3053?ýâ4»8?wI¬…K?ïŸ1Üρæ?ˆ^%×­_?pi/jc ?j@æ?´â?™"û‡¿4Z?¢~!¿©‰ã?í÷§Š|?²veÍÒ?Ú?±OˆyAҌ?«˜Ðù¬?«åXÐIÛ¡?žˆlOÓ_¶?ìÓ¼!¦:?§þí¨?±îµµ"ß?¡Ï™©áo¯?³i9É]?"ði®;-?ëXå<Øy?ž,Õ&Ð?²3H±{‹Ý?"#5×UÑi?hÇ-•SS?" •®´?ïYLVè?ŠX)øüõl?x®KšÄ¥)?q«ÂÁ?­?jh9G?—2h•#?í‹ô'¦ŸÖ?³íÒ¢Té?¯ÿœ^Ä&M?±*ðœ‡K?£i«'ÕH?™p®<3¥?ìå¿>',°?¤$ú/bl|?®:`†Ïþ¶?œ°nfGÚ ?'
,ëTÿ?zØû{u?í'@43Ên?šP©£˜o$?²B¹ÑÓ?˜ÄT—×®šPSR4FGL J1614.1-5047?æf­œc?ǵ|N/7üÀ8ãpOô4À:2ðXõ@ ,3¦¹Ú@IèÄzô?ÊÁPlÕ?Ò(}ˆÁÛ@	²|¤–LÞ@:–ê<Ê6¿ï(å!,u?àכ³¿åWiþ÷Ak¿ä(àwúc¿ïÿðÇô ?ïýçAB?–PSRPSR0FGL J1615.6-5049PSR J1614-50480?ÃÃ]DK*î?¿L·ú¾Þ´?¨Áªk	J?«¾3Áe ?é†"‹<à?Áè _Rî?ºÔÅóu_?»vKŠ²?µ(G¤‡ÈÝ?²òý"~?ê^LïûY?¾LW¡ÁJ?ËUúüh¤b?±sÊé2?ÃÞï;Yå?©P†§ºÉ´?ä2År'î?²; ü®Œ?»æEÀdŹ?žf ç
¤?°ñZ²¿_›?'¹Pš×o.?êeñ-‡Ö?¢•2^†z?´@à"…M?²®ÎKÊP=?ªTíގlõ?±"[¢=,?ëÒ­¦/Ã×?»ªðCV?«Ù­‰ODm?°ŒŸ›àGˆ?À*ŽÒsÞR?ÂÈqŠÿs?ê7Ár{…?ÄC}©àõ?ÁQp±ªÒ?©GqíMãÈ?Äp:"™:­?«ªD°µÊ:?揕Jï+`?²INJ/Ó´?œ•*¿´Dò?†º|%0	_?´îL¥$[7? Rðr+\?ì}ká?¢VÑy58OTHER4FGL J1614.5-2230?æ䧜¼Ž¼@43Ä~I±ûÀ8fé†.ƒÀ;àş±á@ê×™"v?ý™'Í_š?©u}äI?ãMˆÿ˜|
@4f^‰"S?ûq…Þz?ï
–1ÿ?ëP6®è¶7¿Ä9h6¿ãªDâˆõ¿íCçì
õ¿ïÔ»¾²'ÊPSRPSR3FGL J1614.5-2231PSR J1614-2230?Xâz`$Í$?ašEùã?$?'[ÏÜc?vè^
Õh@?'ÃL7¿s™?zŠ	£SÁó?…Çœ¸è&`?îÂ®÷àÞ?¨ˆX3Õ¡?£²"ؽÛh?¦Áà{ÿu"?‰Ð¡Ô·¸û?ŠÅç?ív×Ñsáµ?¢6ȒK3¿?±-8î7?¡cüU†?dq¡¹c>ÿ8~ÊÅT?ïÎ@á'Í‹?ec» 0ä?x²Ç&ht1?eVÊ8?¶?Z¹bM,L?_¤	Ä%?ïÇk&>®?"ËCO_?uœY¼|x?">+ÃâŸ?][K½Z?"2€Ê…?íðÝZtÒ?½KÇ5«í?­ÆÃ^¿?»^­( ;?…–U<SŠš?…zé8ûv?íâaҋ†9?žê–t;µ?¬tM‰ê‡Å?›sz-ë+>ãŠKmBø>âkýc(?ïÈt•?n…[.eÎ?{ôžÝ‹?n?Òö)	PSR4FGL J1615.3-5136?Õ¨ü|׆¿á>Ó°ÜáÀ8Ýñ¸> À:ˆ™|=h@@ *¿;>Åc@¢¡<ü	Ñ?µ°@¥½£?æDí¥Šh¤@&Xn\Ôí-@´€?ï gžÊ°é¿Ô†.B]•¿ÜÜ¥‡äep¿Þ$ò¾#Ñ¿í²
©§-׿ïþÊô<'PSRPSR2FGL J1615.2-5138PSR J1615-5137?LG{…q ?bɬ˜º›?îoË+%âW?²Wn'¢?¨'1ë}>?²ûsÄÁè?x¥"æT ?qv9>!?è¦qÏsÆ?¸¥ýŸ
nY?Ì¡ÿáø?¸©'7j_?'<Zk‰Ð?Ž§0Šc?ë§Pmoˆé?«òÇGÒ§'?¾'mzy:K?©£~†Ùþƒ?P¨¼òRÂ?9O0'o1t?èÊ%¹*·?ª1rc«¾8?Ì·CÊ@f´?ª$&ÖҋÞ?Q2	aŒŸ?KˆÏ®Ø?îà›±Kè?¥˜IWIÙa?¡veøWj?¥~\¥" ?rFKÃ<Ë ?æª2—?é˜9lÞ$¹?À»½¢ðR?ÉçïèÛ¡?ÀŒÃtÕÀ?"É1‡˜'q?'û·}¦?쪄ãÔü?¨1ùýP…ü?¸²¯4Z?¦¿?‡s_?ÑëW©?<îÚÖ¿Ã?êÿ8¶;!$?¯¸±Ÿ»@?Ãÿ9"c°?®þ=³éPSR4FGL J1618.7-4633c¿ìÓ'"Ü…@•ê˜+ÛÀ9=#I±À:©ï§Ã(@p{¥<åä@$º¼)?ÛwNëö]À?×» ¿þˆ1@±+ÿbKO?÷°à]"p?á'‡|a¿â8— B•§¿â[eŠ¿a¿ç™è^x±B¿êg‹"ôk¿×$*í"1PSRpsr2FGL J1619.0-4650PSR J1618-4623*?âà)óÓD?ɔ&˜x»?·8'5dk?µpŽ"+@v?Ôq¢K¼8w?Lj†æ
»?ÑtùÁø]t?ʑÝù)w?ºSy8È?½:þ{?ãûíÎm?ÉÔ+0/r´?Ôî¬qž¹û?²‹m2O¶á?¼¢Ñ2¯w?¥Gœ'ÊM«?áôO Ú´?³&ÊÔý?¦¾<w÷Ö?…í
¯ÜQ$?µÐžÝ^?——U,éSQ?ëÚcƒ?™TΦ?׸s"LR¿?Å­2Ü(èà?ÅH9":N?ÀIÚao?Ý£oßi?ÉL»bŸºù?¹·%¾p?¹Ø'€«êˆ?‡'…?ÂA÷9e"ó?èC.ùgµq?Ä3Ï	?ÇQ3õâ!?©êÈ2I?ÀW_W©_4?©Ì¥§ÈE?æÛ,(+?²ácà)j?Ì§[ΰÆ?k'Ñ Ü}÷?³A'6¯Üª?¥ï$v¾ ?íP›'p?¥ëŠ³9ã-MIXED4FGL J1620.7-4927?äP¶3á·s?ÙâûB+»À6ǎö¨hiÀ:hõ2F¤)@ K6r,@i9™m$? Í¤Ážy?áyß¿î˜@7©)þK?üÁ"À?ïK$£Mx¿Ù¨ââ¸Ç¿ÔÔg ÎN¿ÞØ<'g±¿ì>ß¿Ød¿ïº–ÔÃ;TPSRPSR3FGL J1620.8-4928PSR J1620-4927?ÑK°êË?#Ë+ØÔcÿ?ï~æ锿Ñ?œ>ò%™9?Q‰Æ£ú?œ%>ù›ÿÿ?qõR3Ë?}Š5Ɔò®?ë»P}Q?´€±7½Rÿ?À‹yÐü\\?´{™Þ2ܾ?¾
û>òÓ?‡pÿ|6?íˆ1anQd?¤r

OL4?±†³3A͊?¢€ÏþmtF>´à
a6K.>²¡»lW\—?êâs?~¸χ÷?½8ƒt×'?~·ÜM¥?2ê9 î?3¶)ÕÀ³æ?ï.ü9Ce?—ìLïÇ΋?œïœ¼Î?—Â˼ãgò?fg7¬ÄÃ?t:kIÆ»Å?ì~@!Ù?µ'1X.?º`ÔIK?µY
ïœ?r¯íbSe7?uÖ€_È?î>±:8ú·?Äg²ó†?©¾î¯ùìæ?œ¼yýÎË >€5¸ì')·>"±˜Ãwj?ïÚ˜Ž?€¦o.d?‹ÿySpBó?€¦™CŸÈKPSR4FGL J1623.0-5004?èMÕmk¿Ò©÷þ½áÀ7…J¼Ì¥À:†Œ"ÎX¾@ –üªàéº@Äہ›v?«öÍ&cìä?Ù±y_<{†@%¶å«ÀãŠ@;ùUkí¿ï'½ÂmÎ:?ï|µ«¬¿Ðÿ3ý2›3¿à«;³´M¿éú¿žæàt¿ì^|PSRPSR3FGL J1622.9-5004PSR J1623-5005?^Ôm÷E™'?`>@[J¹?î5'I ãÙ?«ÎªÒ¹ç;?«°7þ‹¥?«#–¶yôð?‡"ðqÕuâ?—²­ç¯Q<?ç]ï9D€?À–Ù	З?ЉNžÚ²O?À!ÉH³Íø?£|‹zsÃÚ?š&íRôܛ?æì4:™?µU¸ÒX¢º?Ïp³Ó½¾?³òv	¥J?d–$µè?P:£æ"•ü?êFã.Á'?§j»D@ ?ƒ=5.?§K'k?bE‡ØSÏ?[:ÉœÚ?îcU!Åw™?¤"UçûíÆ?¨¦Uhâù|?¤ tÊÅE ?yGd)2›ä?€iþ¾Ý?èˆ71¨s?Ä|½© þ±?Íèª!ô?ÄQ	óHâr?šT W}.C?–_Ÿ1dû"?衄âåì?·ŸÐÙ£4?Ê/hm§£H?µxµÆ?>¹:R¨?2Yƒs•?ë‹Çú*(?¨
"ÑJ/Û?ÁÁƒzj̟?¨p©ÁPSR4FGL J1623.0-0315¿Ò256ˆ@>«ÅXdE$À9'˜(€QÊÀ<&‹ÿ}#A@IèVk@3/‡­?³xýlÒ¼%?΅÷eҗ½@@,Meä`@±©'×	'?ïô"'òÜ+¿Ýa=@'¿à)Tݧæc¿â\ä¥5¯¿îvSCsó¿ïÿßÿY'íPSRPSR3FGL J1622.9-0312PSR J1622-0315?ÝÊulò$S?ÄIRU¤è?Ü·«w¯?Åw…væ«	?µ÷³@ù?¥™I•#?ͤ^?a¥ô?ú‰FmÖ%?åž~#`F?Ŝöp_8 ?·Ç/"#Zc?ªö&Öa(Â?á¾iÀ–'/?´á
¸Pû?Ôݵae'?´é²L.?¾•Üqk¹H?¤à,¾ä|£?ÞlKá2"?¦
_Tgå?Ù2ڎ"?§q¸­0û?Ás@ˆ}µ?–"Kð¢?Äɞ!Ç-¯?·ëWæÙ?ç))œ±|?Á"ع-øP?½#vÖåÄ.?±b÷Sۊ°?ÀŸ½þ†`à?Á•7^àO?葈¾€ð?Åljg®v1?º4>>©½?²%!#'ê?ÕŸÖchI?¸ŽÎð€•™?áŽÒì ¥?º3<O^Ž?Á¢…	®nW?ªG\ô˜Zå?ÊÑ*ân?¤ž¢¬ž+?ã0šÛ@·?¯!<íozN?Èn°hNY;?£2¿~‡NÑMIXED4FGL J1624.1-4042?Óð»ª÷¡@©¡N™ÁÀ8P
ýÅÀ;fe€…@w?<ÖÊý@z¼¼´PÕ?©$'bq÷?Û¢‹EC0@)ؽ©CZÉ@8<­…v?ïúeA"_%¿Ñ,}a¡Ì¿à
¯	mg¿æ'"|ú&¢¿ï	OŸz"+¿ïî?CîKPSRPSR3FGL J1624.2-4041PSR J1624-4041?_…±éõ71?b—EpëW)?îÅ	Ca?¨.îc?¢³Aï
O¿?§IïlœÒ?Œëȸ'?¨ÎÈñék?ë\o¯»D?¾)ÚÖ +?À¿"´I'?»ÞZòGŽ=?"Ëç½?'a§²-†˜?ì™äFÚð?§m>ÙÅÞ»?¶>Ñ_;?¤iß:	Q"?rU&Â$í?[D¿¶˜?íŠLÒ
ñ?"7GúF€ä?²ˆGGÁl?""uÖññ?[Qd
?YäÊ4a—?ï;DØ)Ö?ž–²$#!¢?œ¢P+
?<‹h×Är?€»ë'X‡?'΋íJ?êÇßÖÐíÕ?Åa£5F*S?ÃßTæيÃ?ÄÕô©N‡?{þ*C¸?yí¼×šYÖ?í"Ögf|È?£9kfÃgû?²j!ÙYþ?¢^ý\ÿ¸Ç?H¸d®e?5~Fò9%¦?íðöÓ ÿ?"ãSï7Ó"?°H9NDƒ?"ã\áKl·PSR4FGL J1624.3-3952¿Ô@˜»<|@ÃÝ}8ÐÀ9ž3ÆàÀ;ž6`å@'úÇ[ô@üGÿsF?À¾Ëê'Q?Öàþ]ª¨@vì["@æßóÈd?ïý†ì]Œ¿¼vјŽ¸¿Þ5úÀñ¿áË8Bf¬Ý¿ïÿ›‹â ò?ïÞEedÞ§PSRpsr3FGL J1624.2-3957PSR J1624-39?Á'篸P$?²é"ï	?؇}Ô'pC?ÇN¡/²lœ?Þ¯ŽSüg«?Æ 2ÁYK?Ø æ"ÙÄ?ÊÛ	l2?Ð-)î)؅?Â*Ù:¡ð?×±ïŒücz?ÅÅf€Vk`?Í¢y¥f	'?­öVYºÎ?Úÿ)⍺y?±ÅÌOá
?Ö/™J¿@ó?°ç=bŠYx?ޕôc?«³x-‡Ns?ÅÖúÝ;¯? ÿ{†Hæ?Öf~ÄÆ?©Þà NõŸ?²%'p;†?¥/¼+ûíˆ?ÞË¿çß3?ÉõÖ­š	?ܪ܍	=k?ȳÐ>=ʳ?Å&€ÃðìM?ÄDÜÓÖ}?Øƪ[*?'?ÊQ·P—®?ܦBÝJH?ʍÜaˆ?ÀíqEp*=?¥ÓœÛԍÈ?߯E Y?·Ææxô4?؅˜/éÊ?µ¤ŸpÃî?ÈÍÂ^Ì?¤Ü»¢Á?ÐÚ6»0 º?±ëϚ¨$†?á_t0?³¨®nï ,MIXED4FGL J1625.1-0020?ξ$ކ³Ž@?Ö9.÷<À8žÎR
À<CN3iº@3ç}R;6?ý}›6QÌ?§™(c)"Â?áE"žæ_›@1â">iƒ?ýð´`Dc\?Ãa}Uì¿Ï§½^DÙÏ¿ÑÆmãv¿ãwlH'·¿ï¿¼¿ïùM^W¤,PSRPSR3FGL J1625.1-0021PSR J1625-0021?pɵXûc?"¨o?ï»wFLYd?'&{>U?r1"Î&ï?ƒJ[jMî?ƒ}˜§×?f¤ß#å®?î¦è¡‹ø¿?£"ÿ¹? ²2@Ðã? Q‰Ô1ø?ˆe§õ^?Š,eòIÊT?î lõE½?Õé¦Ù:r?§Õ%"—¶?™Wì6ZÁ(?>óçü"°?13¦-Éa?Ø•>?uH3ÞôT?Žå²pù7?tâ
…"@?gñ
BJ‹?tfP0Õk?ïÉpöC?ˆk`ºï™?nyá
)?~§€ð+Ú?€‡´éæ=?h½w§þÎ?î½;vg/?§Á[ØØn£? 
"kÉ¢'?£­pülw¢?~0ŸºWð¦?yöRtÇs6?—ÆŽ?'¶p4³uj?¢ï«>Ê¥‡?'}ê‡4÷Š?kgµÕ"?±'ÚâÙé?ïs4…÷-ý?}ÓþÚN=?'€7Á9%?}Ã¥7ÐPSR4FGL J1627.7+3219¿í,â჊†@EžNaŒâÒÀ:ePÏ%l¡À<»kõò`@1ONFßã?ú¬d\ êÇ?Æn¢ŸýŒ?äv‡*¯@Ì ~$É
?þô¿ÍŠâÈ¿å<ççÛF¿ÛЏ$Äì¿Dr}Ëݹ"¿äج¿f1ã¿ïÿÿ" 5•?ïÿ̾ßú&PSRpsr3FGL J1627.8+3217PSR J1627+3219?Êۇy—?ÈJ–獘Y?è.y c‰?ʂõÆÒH?£.ü$¥½?©É4Ó{?ÆÕüÙ&nÌ?"ïà<,?狑mV?Ä°Âw€·m?µ÷zåî>´?«¥p`1è?ËÕË4W†¶?°Ãa‰tî?äÃÀÅ¿?³—Z[ w ?Áô5¼¥bP?ªÿ8Ÿw·Ä?âƒÙ§·Ð£?²úƒ	ý]M?Ò'ÌMÝÓ?²-HF¯€¥?Á¡njWM? åXGµc^?Äʪ\Ç?ÄRà¸(ò?éfèÊâÅ?ÉSA™[
ö?¬ÎéBy?²"žaõ?±:~BÈsï?±qhD"`Å?êýNŸä?Àw¶÷3¹Ò?¶ÛbÚ¾ô?¸OeÁ@u¾?Â:3| ¼?ª#*ò.÷ˆ?æ¶>¦	u?´ÚæeÜ ?ÂìÑíüzî?°1]		X?Ó¢{{²?µ0äÀ²­Õ?ÚÅgÖÜxÅ?¼=ª¡:?ј­pø!?²³"š'öáMIXED4FGL J1628.1-3204¿Ó).º•@&ûžŒG¡À9>	 '²À<OB]r¢@ú=ºË˜@_'c3?´S~¾].•?ÞÏ·£Dé@!h0Â?«?ögR]šæ?ïôî<‰¿ÙÕRAì3š¿ÝÂž»¿è˜f~9@é¿îÍê¿&¿ïóêþ'PSRPSR3FGL J1628.0-3203PSR J1628-3205?sE•^.R?s´PhJ?îrpà½Ås?¥â¸Äȕ‡?¦p?H¹Y?¤Ó8àfõ'?ŸíyHHø?•ã÷bè>?ìèc´¸âh?´@7­GI¶?µä«}×"?³&±H ¦?ž·ƒ>­Gž?'ߝÝ
F?ê[ê3åàš?¬lX…â‰v?¹fÉ7Áã?©•U"'r?‰GÚ¿f£F?l0bߣ] ?í‰u×óq|?'ÍSöÆG,?°‹Uèå"4?'*·PÉ"?pˆ9F1
?g©1´zgò?îl"b¼Ò?¦ò[ª/Då?§.Œ€–
?¦=JþË?"⸂¤ã?~–
<q?ìlŒæáS ?¾0…U"¶?¹ÿA¶{&?½™%š25?'
/=…F¦?‡È³G›³?ë'c̃%å?­"Ä"Öf?Á Êäþ?«˜ÚÄ슁?b³H
•F?Jå] ô?£?î(Ä¢åP?"ÿÂ'ð?­'?7l`£?"ÙY x]™PSR4FGL J1630.6+3734¿ëª	I@Ešgó
NÀ9ØScTc/À<OÓ7ë)@(¡Ê?©¹?þ"•üV'?¹5Rr=µ?åR›¾aúò@Ì­~«@Oú)ƒ\?ïĬ½bÌ~¿ÖN¾ÿږ9¿ÓÖ¢¤V§¿åˆs¡¸L¿ïÿ÷Ò4Û?ìDÇ_¥'PSRPSR3FGL J1630.2+3733PSR J1630+3734?¯à`o¯Ïâ?«[ ÕAS?í£Vλ0å?¯ïކÉãW?‡¨Êë!?"é"êɆ?¯"ÇOnÙü?¯!Ù܏>u?ì-ÑTÏmÅ?¶$"±hÈ?­Ž#cšI¼?§zå¸üÂP?³€<…ª??£¤"®°?êºaÌ^ùò?«DÐåAU?·q_¦Ÿ5?¢½ Kî?Dz	™H¢?¦.ýÙ?åLÍù?±16eº?ÃîÄT"h?¤Eÿfó— ?–½¨^ÜÃá?–[Ë­½èÙ?ïsrWO6?›ŸC€)?~Ï¥s²IR?}zÌàƒù?—Ô*ƒ!%?šŒÀÄá?텦Cå̽?´–¥–6"?«»†ÎqŸ?±ˆ=ê÷ž?¢¼-&ۊ?˜u}ø¬¹?ì«ï¸ÆA?¤§D°'¶T?±žºiî'7?ž#5ÚÅmd?¨.:*<L^?"S2Û^/í?èäAÖÜh?³Áþ«€Ç?Æcøm9"K?°·5òçOPSR4FGL J1634.7+0235?ëOdÆlû@?T›«–òÀ;p>Ȓ«iÀ=8؆>s@I á÷×=?ÿîóhB¹?Ô¡…‹Å›€?ïüÌnØû¯@(™|=h?øš€Y¦‰?´/ȀÈùj?î$¡ÿ?×ÐÇãÙÙ¦¿æµ¹?§4ã¿ïÿý±q&´?ïÉ+ø¬N¨PSRpsrPSR J1634+02?Ôºœ½ª3ß?Ìm$Ց0X?ãÐÀÈe<£?Îjnœ‹	?­
¦É?¨3'*µ?È8=Çii.?ļÁD‹þ¯?çC.7ο?Æh[œf†$?µv·lÝ1?ªUüC¯mœ?ڍ*8@kÞ?µ¦–y3«?Û¼-"êØH?·šp©Z?ÃmPƒƒ¶6?ªü´›þy?×Kí0œ"?¶D¬Ñcj?âß,t?·Ÿ6m撐?§°d°Z…š?":?]$?Ñe•ÃB¬Å?Ȇ
'˜—³?äúÝE.Í?ËÃNØÄìr?º9Ò€S‰?¶EÛ°?¸`ž)ê?ÂÍ#ý¾ºÄ?êDcà¥?ÈÍFé¸.Ê?µ{iD‰"5?¶'¯\fö?ӆ3Ž€iz?µ‡~"RŒÖ?áWOr.Å?¹ÑýÆ^û?Ö[lƒr?«Ý™E-S?ǟL"Ì?°j3ïÁz{?è›N[ò]ð?¶"å؀lô?´N"Ÿí?£¨©"•Ú‡PSR4FGL J1640.1+2222¿ï'Ö!'Õc@C&³÷+EÀ:É[ÇÎ`À<©'¿9@æ!ƒˆ`6@Úmý3œå?ÆR6X¬"s?Ýd)uDP@úÃ")´@¾OhÈì¿¿ª›©ä@?ïóŠ¦·¿Õ­N ¿ã‡ÕÍÛ@¿ïþg¿Víx¿ã_Ř%%SPSRPSRPSR J1640+2224?ØÒíÿˆ?Ãt$Ñ+è?âL ö?ÃÞu"¹4â?§†ž¯Ìï"?›±^8BÝ7?Û»r©¸+?Śxç]ž?Ý_""Æ?ÅIP(êãl?»"ç
7N?ª‰:Éüú?×ýˆ¸1?µïR@'+?à	C"™?·P¼XéÙ¬?¿¿Ä6âP~?¤?pZ}è?âò _Ë0"?¦_†Õõÿò?Ô\éÁ`n;?§ôŃ:.?¶÷Uû¶Ïr?•$I.žÙ1?Ð'Ȅ‹?½¾9:xË?åøhÉu³?ÁkǓá?¯</DLq?£áÛíE ?ÐQ5I/kJ?ÄÓCç"?ã97{H®?Èm?Ô?Âx·fE7?¶AàŽåO?ɘŠE=Ì¿?²ß½µª2?å€%µ¥á?¸Œ,×}?ÀfáW뛼?©òpýŒL?ӕʕm˜'?«´Jwó‰?á=x†y?³9Ùíç?Ägtó
èÖ?¦U{ܕ"ÚMIXED4FGL J1641.2+8049?çŽxÝÑÔ@?ij=¯øÀ:Ôcb¥ç†À=f{_ï@ªž+#Å,@O–ü0g§?Â;¶šM?Þj'Ûdj8@°4ß۝J?õ;qE< ?ì?i¢[?î§À&KC¿Ý¡<é?t¿è®JáO»ª¿é¨äÅçÖ>¿ïýªë&PSRPSR3FGL J1642.4+8045PSR J1641+8049?ÚâáIÈ?ÊuØÊ1?àUªKÃwä?Ëó–¡RÜ­?±Ç(zËâ½?ªÎ1 À\*?Âä>ÉÐ?Â&Y{FrU?èßë_Vt"?ÃtœÓ"¶?³8vùb€H?§µØ©úºÇ?àÛG~?²±ÇjþŸ¯?Õ·Eø˜é­?²?¾zÝ=?Šò–¯?§fe¾	‹P?Î-AÊ®B&?©°e—l?Z?癶\?hm?«ƒ¹¨?À.?›_&2?Œ®{¸?̸¯Ý0zÐ?Âqbæ ¨9?æÇ©—
£?ÆÞ¨±(p?°QSŠº°J?©yÜÁ×?²·½C!f?À_lˆO«?ë†ôðú è?ÂВßÁ>?±›oð\?ªº¬™é…?ÚhÜÝæûw?µtÉ9F'?ÛÐ*Àù8?·Ë¤Ðý?Íñ°¢?¨I ô1Ä?²Ð+jÖ§?›Zñ!Ǥ:?ìʗ¾£ƒ?£­Ú-Þ_œ?žiÝw™?'ÛåO2ŸMIXED4FGL J1641.2-5317?ÈòïïÀ?\¯-•À8˳;+À;TÚÌiÐ~@=³é@åŸ+©Ò?³²¹¿î†Ë?Üe;µg@"n½	á*R?ÿn±†uO?ïîºþn/‰¿ÔDûb6¿â¦KÄ#°ß¿éKF¿Ä§¿ïýu@ô¼Ö?ïy§4ƒ?PSRPSR3FGL J1641.5-5319PSR J1641-5317?Œjýò+"?‰0#I¶Kd?çÛ²j˜F«?Ã@ G"_1?Îʆv|3,?ÂÝÞÞÙOù?©ÖË4ìþ?µQO¯;?å¨ôDNÓ?Ãà|ƾڋ?҇í=õGÚ?Á8ª$›Á?¬ûgŽq?œ"Ú
qÛ?ç˜h²y—ú?³¤öÙùv?Ê_ƒPàuÕ?²^Nš
æ`?¯½š3U>Œ?"b"¦™?äމÊ]u–?®ÂFÉÙv€?ÒK9#ã	$?«Êš¥T°(?–÷Z81?«|JGY­?睈6Dà…?ëZè•"?ÎÈ:ɐ¾?»‹¼Œ7Ü?•c"´° o?¬xRɑß?æ'Ø"?Ç´¦6V.?хÁ}ÚÓ?Æw†ÒË&?›²¯¡/õ?­Šm?èßöëâÅ:?µ|:íâ}*?É	ҚIËY?´PÍrÆ
?‹¼xÅ"YR?w.ÄÏ(x?æC%w*P?´£PJYæ1?қáïu?´㾗/%PSR4FGL J1648.4-4611?林g%S!¿éÏ]Àû]YÀ7ÄfUŸnÆÀ:b¸[ü€@ 1)ÆMå@£¢Y[»è?°áà°.†{?Þ9ÚÙ)ý@$ê ¼8*@pjKM[?èY}êçj¿àÌö¡¿Ë¥ô[\6¿áڕwËéx¿ëbšÿË&Ú¿ëDLˊ­nPSRPSR3FGL J1648.3-4611PSR J1648-4611?hŒ!¨$¯?xv*•'?îñ.._?'¼‡d ¯?žÎHŸlqŒ?šÑ<½{ò?†Jûn#]Î?Ü××£Þ?çU c«S´?¾'+,ÃFU?Уg]Ý*é?½Åɧ˜#½?ªÆТY®?Ÿ¤ûú—Y?èp­Q²OH?±´-xñôÉ?Nj–iˆô?°DÉ=v-.?rXoZ9]?Y®éi;?æë@͜ù?¬côfܽ?ÓªÇÀY³?«îRòTìw?ƒÙ(6C€?±‡Ê0²œÂ?îâ}1Gå?±äגÝïˆ?™Ò¼7艹?';¡' u#?zcmÚA^(?K¥£?ç'Õ:.¥?ÈÚځ–C?ÐrÇÔ{¨ÿ?Ã_V3Ø'?ž0$¨.q}?–0ÒI?êŸ3:Ù´?­™Ï=x-$?Á½.~îr?«)0z'§?H?d¤,`)?7«÷–Mx?ç×:¿®è?°&ƒÇ¿)ž?ÐElJîW?°"¡ÍgéPSR4FGL J1649.8-3010?ï¾¾ì†ÈÔ@"lQ¹07ÖÀ9`òl™†NÀ;ë]"ðÅÐ@I í¶Q@§ºÄŒŒk?¹"ù¼o?ݞPõùl@ ™÷L¿éñ8ŸXËH?ï¢ý$ƒm¿ãÑàd)u¿ÚºûéðÊ¿ã@Bæ.ž¿ïÿþˆ0»Š¿ë·é íö¾PSRpsr3FGL J1649.6-3007PSR J1649-3012?¦'Ë‹·?·µ>?íûu+Ñ/?¹±]ÆÚÖ?"‹Ãp—<©?™§Ç^í®ì?ƒÆ¢Ý)W8?"ݝÀÊÔÞ?ë$ÓÞ¹?—F½'Ü?Â0I£%ù(?ÂGIËPþ?¸nL…
Ø?¤æ)ëæâZ?椆ŠÑ³D?°ÕŒ¹ ?É6¿QÀE?¬š<&­Ûô?VŠÌO¸ö?@Bð"»äl?î ôŠ^œ?"O/-¹"€?­ñä`±}?"
d2³? ˜Óû"?³˜Gnyˆ?î1*úš2?¶NÍ,«ö?˜ª6þ§? -2?Ò¯¹?ƒ ×ãl¦?›š,°oñk?êr/g4w?Éø9ùÔu?Å4æDJ»?ÉÝ+X$?®">HÕ?¡f{å]û?è»4P˜?²—¶ =+<?ÅoÉð7ì?¯†ædq›?6¹Z'Æøò?&eôRE‹)?t?œyaÕWìÃ?­è¬^9¾Š?œfäMu¡PSR4FGL J1650.3-4600?ìÝÖº}¿î€ž@GmÓÀ7¬r•;fÀ:GÏASC@80Fé@bO̲+?²N×>ã'?ÞÁ»=j@&–V«Þ?¼@RÞ³T*Ð?ÜÇ<? |L?Ë¥ñÁ£ÎÒ¿à4äv]¿å½‹±yŠ0¿îø/¼†-¬¿éœŽ i¬íPSRPSR3FGL J1650.3-4600PSR J1650-4601?f	҆?e D©ŠK?ítÄä‡9×?´ú€è‡c?³©¨'os?´Xá²y9?ƒ:†šSŸÛ?‹Èំ‡]?éƒû]Úý?µº?Ã+¼±?ȼkD‹d?µ™nh4ê?M"G¨‹?–&ôډ®'?ér¡¦6¿?²D÷eXž?ƑÃñ °?°¡ì}C?N¸MßDZ#?6?uqîq?éoהYœ\?¡˜VjÈ?Ê!é`ùŒk?¡'°BÌ?a-_÷œ?VГšíÒº?ìk¶6Þ8…?·— ‰y›4?¼¥Øí™?·zÂá3®?s¤{rƒªk?yÐfó¶·?ê`H3Y?¹ÞoÙÏ8?Åâ×
	?¹¿[äÇN?'0 ps;©?mžªTƺ?ê~OL›¨?²vϖƒ?ÃÀ®Àak?±«×ðÓxt?!ž‰¡??Î}u^Fr?ë
	&Uf?¤Ýaâ?Ãǔ@`º¢?¤ˆ¸úÈPSR4FGL J1653.6-0158¿ãÀâ̓ðª@8ñˆÁÛCÀ8Yˆ1'IÀ;ˆ×§b\@ÕºǬ@‹ôÄü?¤gÉ<õSÕ?Ñí×ßO†P@+ÂÑ(| @Åìäo"?™žõµ5¿ÕÀáÜÿIø¿â£ÿYçÓ¿ç÷Í+—]¿î¢Î–Ñh=¿ïþ'MKã-PSRPSR3FGL J1653.6-0158PSR J1653-0158?"ˆE%ÿd?€5oÞí.??ííS›2¡?¨hš÷¢?¬)h´=lš?¦3nhÖh?'ט‰¢vO?™}75öµ?î7ŠZâO?ªƒ¸A0" ?¥Ð»ñ?£¥¶¯2?²žäxüET?£®F×)ó?êG.B¼Ö?°‰¬Â!ja?»'©t$Œt?§Àõà3N?…šà¥ùw›?qvjÄ߸v?ì¸-E)ø?™£VíÞ¦?·‹9À9BK?—–><ɇ?}`^E¢Ïã?w=ãþ©&?î'R¸Å¿ù?­(Tf,Û?©ÞÈ­gê?«ô^†$1?‰ÂÚ{'?•Ñ#˜–?îr¨ˆÂ(P?©MQéíõ?¢dÀð†Ìt?¢°fªLýÜ?žÒwÍ>—?˜¤‰Û¸,j?ì–¤Fƹ?«Eß.åv?·î¬ëÏÕ?¦û±ìÀ•Ù?iû'õFÖ?\;a¢SÉÎ?ìoÿ1N¿?¢7ÏsFþÕ?»°)ÜzóD?¡å<CøßBPSR4FGL J1658.6-5323¿ÒGm3×jWÀv/¾3¬ÖÀ8¥èYM‰À;š
oTK²@$$5>{@<§…ëfì?®¢Ç{æ;š?àæ
Î&"@)¨U•:@u—†ÄÖ¿Ó¼¢}méè?¨­1žU™¿ãaΆá01¿ê¥)Ô½\¿ïÿ÷fÔJp?¡j£	#PSRPSR3FGL J1658.4-5323PSR J1658-5324?˜ç$aH?ž.0­…Š?ëïQêXxè?¿‰Okð`r?ºKªbê…ð?º¾‹|±'›?'&ÿ¼ä? A³Œ~?è؛5ɼ?½ÚåÝÚ?Êxиâ³?½ï6•N—y?±Ë0&¦l?¢i,\×J?êȅÈßá?¯"Ù>´Át?½>¹¤&‰?¨€.â³Â?‡â{4ԝü?r¯ÒFX†Ù?íHIoàŽ?—™¨­™è?´énLœU?–ã݉è?•0S@*"Ï?"&Äà¦:À?ë¤5åü/?¾Çì	ËRF?Ád¿Oê,?»|N£.ÌO?Šæà¼qI"?™Ž*×mZd?éÐã™?ÅJ/«nâ?Ê9R´$VÄ?Ä|X'Í®…? ç@5b(?–f¤ڎÃ?ëŒ4|ð|»?ªó¬/g?»*»ü+ ?¦3^^?\Ä[ø@ô]?LO¡y•A
?휳ü‹??œAª¢ÞðC?²§N­\û÷?œØézRcPSR4FGL J1702.9-4131?äíYý:©?´Ûö5{âÏÀ8t™ŸxÖ«À:=
:{&@vRëŠR)@Æ
c0Q?Ãӑ·øÕ>?á=;•"d@·²ôݍ?þn©›z?£‰£édï?ï ^¿Óêù¿Ý·âYü˘¿ê‰œ*Œñ¿ïÿ§J\D¤?ïïùø?PSRPSRPSR J1702-4128?§ìˆlà"÷?¯ÄËÛçñ?éÎϋó?Çܯgzý;?Â̪¦dáµ?ÅD\Xùõ?ª?JÒ7û?²øó'ö?Ü%jC{æç?ÅB˜\õ¾?àIV1~Áì?ŕ|,æê?Â{.â
A?­¨M¦ ò†?ԉä†c8?³3K/Iè?áBK-?´I˜0în?‹OàU$P–?p©{ʵË?Ýðd^Ç?±¿´xj?áHxP?±§Èüˆ§.?•&/	oúÁ?°;덉Z?êÛó§"=›?Ęç&.+Ñ?Áëk€N|?²¶ºÖnü?‰
©ì
Y?"1þ!Oþ<?àd2D©Zà?ÍJ!ÕEtÝ?Þo.'ÿ­?Í2@U@à?¶§>‹z?¥£½¾h»?×,)Vïµ?·ž¿‡åž?á•'sÊ?¸J³]‰×?a¨8:¨vB?N"s"¶$?ᆺ}P?¹A…Ⱦì?ÜÏ:•¨k?¹-\D²3MIXED4FGL J1705.6-1909¿ïÿþ Y|H@)ý‡ÂÁÀ:7/p0ÄÀ<O!Æ#e`@ÌiiP@;ªe™·Í?α%|fWù?ïþx
Ә™@媴ts?ùùu$dÖ?ïòù¢í]?×S"ÜùÀ¡¿âànrb¿ëå#¿¸è¿ê^ëÈRj¿ïÿYM»PSRPSRPSR J1705-1906?·KsN‰Ùf?¾t:JºÊ}?çÝ}|º?ÍDápó³?ÄäR
Êðe?ě¥o]'p?¯H|䊷1?·S©X{?ê"s¦¯›}?Án3ïñ•?¼8$Vÿ?·ˆ¯&‹¿m?×+¢Ê^¢<?³šÁªe?ØG4è%ý?³M9˜ÍÍÆ?Ѝ(M7È?¯óO‰F?š'¶$Õýl?'÷ib(?ízèùÿ
?š«µ;eТ?«P8Š?•¢ðiæÌÉ?¦Ä2ëBa?©8è"e?çkôš¤º?ÉÂ.Æ"Ö?Ì¢{_Ç»Á?ǐ`zn±?¡ÅÔÔæÉ9?±dܲŒÉk?ë0߯07^?ÅÑ{£î?½–Sw?Áƒsü@?Ð~ÈÀ<Š?°.',<4i?ÝÍôêù¾?³ø…ø9þx?Ñ´LF»·?±Uhþv\?pæDØûú?dÝ,M1R[?îg…žK@?ž[X!qm??§qŸ	"¾?œÉn´%§PSR4FGL J1709.7-4429¿é-hGß_À~DÄU/À4h1†:À9qŒ;E‰@&ôî)ô@ÚZæÖc?y5£ •?ÑyQ…XÄè@T8sWæpã@†MZý?¿Q~wÕ$¿Ð›YÂéôü¿ßt†¥ 5€¿ãáû2:寿ë£Q^‹³¿îs'i#°PSRPSR3FGL J1709.7-4429PSR J1709-4429?@G³]nX?W)І‡B{?íFφªBx?¶ô¾Q¤¸?µ¨ôdó?¶àÈ0ŸžÛ?"7ò¶œƒâ?°#'+ÐÙÆ?îýCecÌ?²âÔÇ;?&?–;™ú‹£—?¤J¨`U?›u~ê*|?™mĝŒ?éƒ÷oÒd«?²R¸ÎÄòÙ?Ɓ~°4:Å?°
ÎðP{<µº1)¥X<äé¤Ï@¦?ïÿ{â4Ï&?$àü~q@?ƒ³]óÐx?$àü~q@?@§'Vf?7RÍþ6:?íOªôF?¸·R%t€F?·4·±¥?¸°"Ë3ù	?r¦š¯&r?'G
ۚ'Û?ï] •Tn?§	O¬]
?©‡RŽ%?¤æó˜e'?ƒ´?EÍ?ˆr÷äëŒ?ë¨
<¼@Z?°k	*¤ƒ?À$•Ç¹"Ý?®"škъL<ÇmÅä")ö=§<Ü›ù?ïú?ë8®Ù?h~sŸö/;?GS:ýú?h~sŸö/;PSR4FGL J1713.8+0747¿ì[@Lßt@95Ïþ°t§À9­¯j¼6}À<9HW‡¦R@"»ß@î?ý@YŒcP?·"~ޓ"é?á<ñvu¨@ Áòº`@NJƒ&:§?îpOô4ã?¿'ð]À»¿Ä£Ï½íáÅ¿âí ßôq׿îúS] ;¿ïú­z÷íãPSRPSR3FGL J1714.0+0748PSR J1713+0747?‹F?oû'<?$Áç|·?ïhþÐ;Rx?"9Ìòé'?tôú ¼?tƶ"Ë|?›Uüþò"˜?ž«7Â2@Ï?í˜..€?©Àà½<‡?¨Ô°í­?£›®ü,.?›æûB×?"¬³#"?í7
êÒ? Bxüd@Ò?©"+s?˜ëÊhïX?¶Ð†ãb?•5éüˆ»?èYòå=?¥œKS$:(?ÂbTÂé¸Û?ž¶óžR"þ?‡½ë›C?…Ru1Ÿ#5?ïoÚoš?!æÑþx?x—)ziQú?z'F=ð‡,?Y:K-åf?'·,FÍ?î5íûÏ!n?¥éÜAÓ²?¤ÊÑ­®ºÃ? !`'©úÕ?ŠÕ4Ñù?'©,ÿÓb{?îÆkxŽ?—w0d× ?§"îLøÝ?"Åep	aÚ?ÈõRŸW?")ÅÞ4t?éóg)ɗ?«(Õ\#?Äz D®…º?¨SJ–+nüPSR4FGL J1714.4-3830¿îã[TÃ~?¾óÙ@£‰2À7_Ÿ¢ÈÀ9¿¬aó:@ –lŠÂ¼(@"=ÚV"L?¬÷ÃhcÛ?Ç1Ubˆ
{@¡\Á¡ö_?ú|ePç¤?ïééªS%¿ÚŒÉÝ.Cà¿áŸ—£ö¿åô¯iå¿é+܂!'Ý¿ç×ó;Ì^éPSRPSR2FGL J1714.5-3829PSR J1714-3830?'_¾Gü?'q£Ýõ|	?ÇKªMq?ŽÃÐ#ïH?é¥Áû/C?Æ$)H+pz?| Põ{?çG…!Ræ?Ü8óçmâÝ?ÉÀ^#¾S?á«^Ëgqÿ?Éó€¤Äß²?­üäjîÎ?ž¥K·~/?ÈÊ®ÖRî¡?±a[¿JV†?çüd|Mл?²n9qXß?[Ň)ó£	?B¢M†S?Ôʕ\j†?¬\-P»ÇP?åê7ò	È+?¬Y{GN<1?'€QÀ°>?}úwM¾ù?ÒT—'¤EÖ?Çï'ÄÙÓ	?拶=O|ü?Çó2bäâÔ?s–J«‡E?r(ڞUn?Þ›0ÑÔ?ÏZÿ]¡N?àÐÒZˆë?ψ"j‰?¤ÂÖÆúŸ?™	|'¥k?ÉfÀ¼¦Â€?¶ $VABO?èZ"d¨6?¶éÒìLÖ?4Þ*ÝËíÇ?#WÇ×÷>?Øc@«ÊQ?´`ñÚ8Ë?ãË֚Mk?´^Ž‹á"œOTHER4FGL J1718.2-3825¿ï*c‹•Ÿå¿ÜH%EáÀ7	hQ"1ƒÀ:0«¼²@'ã»-h@ÎåD'×?¦(Öbø¶?ÖÃê¥û¨@-Tšþ§±?ñü^]-'š?ïš ri¿×Ÿ2à§õþ¿ä± Hõ½¿ç+
=²é¿îFY¶T»C¿îNõѨԠPSRPSR3FGL J1718.1-3825PSR J1718-3825?t]½vË¿Ù? I*˜g?íä·K™?²0`$jß?¯(ØHMn?°A<YyM\?uƒ^o{%Ï?ê¡ê6?êJžV¯h?¶¿·fcUH?Æ)k²Xó?¶ª/Þ§Ü!?šC|u/¡?•æ­Zs[?é™Õ¶?±«…³Á_?ÆP<eXkÉ?°uëóyL?|™7ö2.>óÈá®Óû?ìýLú½?šôÕ«[?¸Vvß?šô!T­d#?d"WÄ5Ç1?Ž'"³'?ìϸi_â`?¸™ûÆuÊÑ?¸Ý¡õøY?¸3XEÊ=?p¤ÂC¾:?x憈£Ë?êáVo€ôæ?¼ßPÄ#í?Ãõ€0x)?»ø 'ߪº?—s‡]Ã?Ž7C?¯h?êÒQ¿mò*?²Q»N¬'¿?¶¦iX"?±vH)y>Κc•ìÃÊ>ȖXC›X?íîÁ|•0?›oJªb˜?±âLÀ~Þù?›o/aLyPSR4FGL J1720.8-1937?º¸³æ!¶@#‡ÔCédÀ:!4AP,hÀ;´%ï@zîüÍpŒ@ÏBBš¯C?ÊËúêÂV?¾Ê°'Úb¸?÷â™7t
"@¾P7¥Þ¡?ïü6¢(‰a?Ë^7u¦¿êR®ž8¾¿Û`·õ¥3¿æñX½†]Ó¿ïõ=~æìPSRpsrPSR J1721-1936?â¥Yoÿ?Æ|['šC?e"ÍVÿMû?`âu1ۜU?Û͍³BžF?Æp¤"À?ìKoéhJ?´N<-j¸?~CÑ´e¿L?x̵:	h?»ÀJfP9?³£Õ¤æ"?éܲ\wéà?¬À†ü´?zK—ûVD?ƒÆÖ·–?Æ}íø?ªâ ­5âù?ëÞ
øø5?'»-R£Ï?•h°ÃÊp?r`ý5S?»µd]ä¯?Z|gŠC?ØDkLݱÕ?•Sƞÿ?vŠî(7¼»?qf"è¶N?ã°´}Bt?§½`j›L?æú	I»ñï?Å­¡ž¾û?ŒÆ{5;²D?HÿÄK?Ñ%¹'Þ>?ÅDª^¸È?ℹfyÂË?µð§«&Ë?¡ž¼cá
?ÙJúô)<?ØÔ9\[åH?µ'"›ÅÊ£?æk¾¿eR?¤Ê->?§Gò4ŸË¶?Œ@Š:ª@ž?Ð?":óØ?£9þ(ÌMIXED4FGL J1728.1-1610¿è˜²è¹×@$`;ÄÒ,ˆÀ:S'ŠŸbÀ;ðaXàkæ@³àúVGà@ê%Ðt!?×0y@?å¨Íê>y@/À_A?þ—ÌLÊ3?ØwGà{ˆ?ïôà²\Þþ¿Ä
8èÿ³T¿çÙÁ§Õœ¿ïÿûbâMh?ïÿ<Uñ¤PSRpsrPSR J1727-1609?À &ñÈÛ?¸èד{ý?è0Îl½¡?Ä)ñ#@Þ?½9@d/e¯?ºØ§=Î?Հ^c|jù?Ð2M§uØ?ÞwÌ[I
 ?ÏB;}žU/?Ȫ'uÌ?Âr^$3Í?҃l}ùøK?±rT}¨Û?Ú5G?³ ô»U
†?ÓG"iíÀž?°vÃNögŽ?ÅëTyvZó?¥îÄï2Ó<?âÃóXìo?³v®ðš?ÏÞ"×è¬?°ޙæ¶ý?¯!"`…âê?§ë*öl¼?é>†ö O£?Ãz´¤ëdñ?Ã=]H¹?Á~7ŠÓ%?Ã.¦"tˆà?È"–ÃH?äþDÞ+o?Ïyºi{wM?ÈÙHYÉd?Ä´M=å-?ÈQ"µw?«œžÂßtU?ß_]Ò²Ù ?¶褣ö°?Ԙyjò^¤?³wþÎÿ6?¥—H	«'?'Mœ(Ïõ?äq"úG¦ª?Átþ9V?Ôj≺?Àߔô¨gPSR4FGL J1730.5-3352¿äßøVF?°ÎÃG
IÀ7⺎ç¡À9Ú׊•ð˜@j±UXL@½ÀÛ'£?¾»+ÿQC?Ò܌=:ž@<ewS@H)Âq)8?îúæ ³iN¿ã5'»0¿åÞv½÷qç¿éª<P¿ê‡¡8¿ïõ|RÆPSRPSR2FGL J1730.5-3350PSR J1730-3350?¨œ¤øÁ¸?¥•`%â?Ó±{í% »?É 7'[?äw¹íC‡?É‹•º?ŸÈ^™Œ…>?¡@UÛ~ÁQ?ÈýR»cÄ?¶ÝÊé T.?èÂ|¶MÉ%?¸åÞõ!?¶ikiî?£î[XdqÏ?ÃÉ«ôÔÂ~?«Âஹ¸ß?èMGÕgâ#?°þÁ¬":c?ƒw[ŠÎþ;?dÐhbgò¹?ÅÐe*­1?œi¾çZ7q?ê>	GsÔ[?œál2ù?–4žáw‰?¥È,ò)è,?ܸ~lþ—0?Ì3n=0ž??àòÙOg?ÌC
LTþp?‹½KŠu˜?'Vì*¢?ÇVu¼‰w|?»9wk­‰L?é»nKjÀ?»$_
Š4Õ?°4ñZÕ÷^? Jå°¸2ü?ř,…ÞÀ"?±­ÞKl"f?è"³҃?´¸7Ès?_´rkŠñ?GÒÀ^Àit?̬¾?ýW??¨¹È/¦ƒ.?èÄö6¨ˆ ?¨¾Jð<‰5OTHER4FGL J1730.8-2303¿ïî—óÚ¶M@ÇŸ¾vÉÀ9£@4£vÀ;AÜ@W@†ž^ÐDü@(3àØŒ?ÉÓËñÛz?áRíãÉª@;ç)oe@yÙú1ßÌ?ïItR¸3¹?ïÚyޓHÈ¿ä3ÞSÝοë
`z"¿ïþBžHU¿ïøT¥sÂoPSRPSRPSR J1730-2304?×ØZ|ÎU?Ã]‰†Y©r?ÔÏ #¶éa?ĎÖOµþ]?ÓX…aB)	?ÃE
'}>ç?Àûƒ¦_?ÂiËqi5	?ߞPOE/?ÊNmã՟Q?×ãí݋t?Å3³3§*?Õ%ÜJ:®?°Ycy›#<?Ëq
<I?®ÓT	ôHÝ?ÝKë0:/|?³JÑGvZQ?´Se"W±?'@(ž‹š?âìK8ž¾-?±Ð¶|@|Ï?Ր)ÈE?°¹PÅʍ?¾SŠ8íK?°¼5˜ƒ¾?àôS¨¯¦?ÈÇIU3Ž"?ւ" ea?Æ»ºò•ðS?«ÓäÚdÙ×?´¨ÆtæSS?á*ÊXÿ°?Ό²Ë™Ææ?Ú/î³Z¤?Ëýu1ìrk?ÈÍ«¦ÙÀs?«+7,»?Ÿ?Ï&Û¨?²­y– ²?â߅¥á?µŒ¡H:n?',û'†JŸ?x¡àî"?åÕ9»É<?¶)¥¼xÒá?ÓB¼ÁD‹ÿ?µw¾
eoüMIXED4FGL J1731.7-1850?éüýùs'@ ÂÀð À:;ô¢ÕÀ;ÐÔÚ¸GÛ@öÀ l8@­±™jŸ±?ÎðʐÀW?æ¿Û¢¨‹û@­¢™ó\@(ÿ#·T?ïõ桊(ã¿ââ÷Fÿä6"¡¸!¿íÅWïnb¿î¬ ‡t~¿ïPk®ŒpPSRpsrPSR J1731-1847?Æò¿²îø?½šQd÷{w?»òŠ(ã?´L£Ó3.?æÄþî÷³Å?ÂÐÒÖQ/ó?ÕÍ.Çh´Ê?ÆÍë"ÒÏ4?Ѿ'‡"?Á"ðèž?Øt>±·!?ûH!?áömÙ]?±ñ̃ÖÙ?Âã* (Ù,?¥´ùÅ8??Ò¡=0sL?®°ˆ''Ì?۔3ï`Ô?¤Ä]Ä×5?ÒH æÁ?¤›"äØfœ?Ò#/Z
¸k?¢d§Rør?³›.áh0?­‹ M0?½Ê#­·¼M?µ±"µ©Q?éÓU­å¶?½£­6âó³?őËåM8?Ãräùê<I?×ÚYîÞ?ÉbŒUýý?Ý\ÀjS†?ÈúÁ>p s?Ö¢jÙ<Dz?²Fä9'?Êu—ò$ ?°­í%Â8H?Ü"É-°è@?µ€¼…?ÆGi'*?¢'ÿyL'?ÙèiªqG?²ÖŒ(jð?ÚóáïHͤ?±}¸
ʔMIXED4FGL J1732.5-3131¿Ð5°œÑ˜ ?ðã†Lµ»À6ioê›ëÀ:oE	@OÁ^Z@|¢}méè?˜‰:%ë¢?ã/џ‹A@A㦽nŠø?ûȚ$W"?ïáKª"}Ù?Ðxoþ?¶y¿ÑZ³ɹȿãÔÐ=0ã¿î.Ö­ _¿îË¥»PSRPSR3FGL J1732.5-3130PSR J1732-3131?ò+iš¼?ðšH†N?ïÛÇ£º|5?ozÀIˆH?qúIʳÉÅ?oU%j­{Ù?m™4¸Ò¢?×ɋòH?íß²p]¾«?±êÓ5+6ä?°¢Ö¦Œ¿?±•Í.·òw?tù–æS4?}(öêe¸Ž?íúA|C"Í? k¾mx#^?­¼µ\֋6?Ÿî¬y"ß1>-yE>÷Ý>9jzLRº?ïô*jéÇ?RUy€µÍ?W«''	—I?RT™¶þ?5ÊR?$-
;?ï֌Cš?qµ´:?t_<'ÛÔ	?qbï`ºó¹?]ƒàÜ:?oó'´Ü©?îá~n[?ªÔ^(¹¹s?¡Ü0!g?ªkVæÉ?nù|g¶pà?naÚ½ôí?îaHÑd?™]{<S›È?§ûÛ'4už?˜Üeñ÷S´=ú%ò—ë´U>–œò;…?ïñ®Ãø<è?[½}f?\¢w6^á?[½}xëùPSR4FGL J1732.7-5050?è6jÀñªÛÀ"énX£/EÀ9×ò<ÉÀ<2³àl¼Â@·(@7`9%»{?»UJ	c?Ôßs㧄¿@¢;ÿŠ@ôöw5F?ïø€_5ð}?—Ä֚g¿Þ|RáÏ=j¿ã®ŠÂfA}¿ï7iÃèø|¿œ}ãä*ÁPSRPSR3FGL J1732.5-5048PSR J1732-5049?ãkՌAŸæ?ÄwÕ0•ì]?ÑÔní¥,?ÂG¸ÆŽ?½O—é|l?«Ž{]\œ?ÞóÈÜt¬ó?Ì÷38ø«3?úV(Î?¾VÓêUý@?×/ äjè?ÇÀìYZi?àÉZ@W"?µ9Ŕ6gÍ?Ö,­nHï?³ANJ«…£?À<"š?©4Ÿ´"º6?ê=ˆJ"I?›íG¦
Ą?½Ú'=vûV?–Ÿ–ê¯å?°9,rSù_?þcj*»?ØøeæJ?Ą
\E6|?ÝE|Öã?ö'ÙaÓ?Ãée
9¾,?²:õÛ#ë?ӖoÔµ_¯?ËvkŠEFd?Ì£òƒÈ?Ægh=šÙú?Þ
²	í?Ëj4§& ?Øÿæ¹K?¶úVšûÁ?ÜE.¡C?·ï_yÜ;µ?ÅwµÕJ°ä?¬Êë÷	ŒF?á*j3lˆ?¬Þ¿ cc?ÓÓ>«âF‡?¯Rp݅#7?ïÙÛíÀÒ?¤ô"Ö°'/MIXED4FGL J1739.4-3015?ïü£ë@?Üã!M»À8¤i×4/À:†ð¬¥åØ@øèë¡@âEõ­–§?Ä_|sp?ä÷—{²(@¿ï|$=Í@nCG'†Ø¿ïЅžºë¤?ïüúz…¿Ù#faˆÜ¿ê@þB:¸
¿í¸^_Ö¿ïÿì´É ÈPSRPSRPSR J1739-3023?¯>þŸVÈ?´µ¾ÊGå±?èC"KÉO?ÍqŸyc£?dz2bÕ?È'â`÷€?¢U?Ÿ¯?°Îªý£]?á‰Yæ%cg?Å%Ï¥ø«+?Úªá‹ÜÓ¼?Äjyà/™å?½ð€V㢸?§/'7ý&Å?߀P¤Õ"N?´ìÄ&r÷?ُEq"?³
tÙ äŸ?ârMØY?zÒèؤ?àéW(þt?®Àûá¡ëÚ?ÜO*‰…>2?­þ¶;?–J©š¹Ad?šˆ#'Ù?麎-Ø^?ÅEÌà:_?ÆLr‡º|œ?û€üçƒ?ŽOäøET&?¨ ;o"ê¿?åbWÆe?È|ßψéÉ?ÔIj³ŽH"?ÈQ"bç'?³`À2€H?¢µN=0ï?ᎆP%÷?¸Ú^Š׸?ØÍnà?·:mL$??{dqÖoB?b'+ä>iV?ã¼gÅ7l?´wÀ©lº?Øž®ùŸ‹?´MÁb¯yPSR4FGL J1740.5+1005¿íPœœû›@4EèÄzôÀ:ý©äjxÀ;ص–Ob>@Ìò"l`Ñ@"à??Æj©V¥ÿ?ÉF…àÕt?ú˜äÓSϋ?ücñ9Æ+?ïýÞ½ç¿åԅ=l3¿ìÊAR¿â&H3uxR¿ïútpe¿ïŽhþÇÜPSRPSRPSR J1740+1000?î¶íÛm×ý?£‹·"èk?€#°VÇÿ]?vðÔaÁ9? ˆ64Ž_Ñ?¢{ó?£+?ës'dÁ˒?Ã>ûÕñ0&?²ÉQµ?ºÈ÷ÄáàŸ?±šnº·>?´mÀÙS·Æ?ë…'ŒÆ3?§í´µë?¤8k³®¾?–™Æü¼?½gÞwÅ	?¤¦³ø.i?èd˜ôEÕ?ü±â}Ȋ?¹Iý7T1?•$š'1?Áȝ"#]Ó?–ú\-üˆ>?ÆwÀ?§Úó§¾0¹?<sñ
ç?‰P«ÒRß?§F7‡UÊ7?¥¨L82Ž'?æX'f'.÷?É®æ™è?ÅT"·:w?Å7©'«°ë?ÁI"°)0®?»e	'p¢¢?ç-¤ªˆ™?°¤ÆM ª'?¶%¢Ðõ²f?¢‹Ö¢äq?È6›ï¶?«Œ"ÝDË(?Ýï€DÍ©?­£0^Q ?Ð)½ëˆz?°É«És±;?ÒÅrÀ¼É?¬(֖'ÁnAGN4FGL J1741.4+1354?ï.@3"ý@5«ä›«—À:5òý¸ýãÀ<O)õœÏ¯@å7¿)Ì?ÿ±a‡"à?Á¥[Ä¡Û?Ü	`{ë´@ .s±?þ©l$ìH"¿Í®Ñd65q¿à³xgðª¿Ò3Ðý^*¿åIåý{¿ìË`P¢¯Ã¿ïÿê0ŠâGPSRPSR3FGL J1741.5+1351PSR J1741+1351?Õðˆ¡­Aö?ð	8Ÿ?â'WŒ•
z?Æ,Á"QJ?³³!~‹Y?¦›^ù\8?ÖhßÄî~p?Ça¨³à93?á§':ÚÚ?È^"¯hҖ?¹#GG"u?«L1ŸÉÚ5?Í|åÜ
?°³—,{	ì?ãªkc{O'?´Õ£ãƒúI?ÃÙmb6´{?¨l«Ñ‰ÝÕ?ãI7"ÊZŠ?¤*(憺Í?Î:Þ"_¦Y?¡T‹w¶Ô?Ä CŠvï~?˜ñ¢"?Ô?Ã/P¿Nù§?µÒ!ó¶>Ã?è2¯žØaš?¾ð2(Ws@?¸áŒÄÁ]?­avë²?ÅA×tà@Œ?Á˜4Gbóž?çt>/)}?Æ4Á9?¼¯$Æ3?²ñËÄ@
?Àµ_ÂÍ?«BÝN"û?çX™¥"4ç?´þ•¸Ÿªf?Áè‡	ì_\?¬>û8Q?Õ÷¯ïÀ?¬*iyÚü?Ø…M\T?±>¹Þý^¸?ÑîáÌ°"ª?¨&ŒMIXED4FGL J1741.9-2054?ﬤßPš@Ÿ@=ݱ!À6äN¼üÀ:Á±RóÂÛ@%'cœ1¤@)õ>ÛÝâ?š¢x²¼?è
U¾xv3@C¿ohی?þa3™Š€!?íúՉ3ðÈ¿Ì8èê9Å¿âOÅÀi<¿íu!À5¿ïÿ¹žœ¸³¿ïÝ6LJ[PSRPSR3FGL J1741.9-2054PSR J1741-2054?",˜I¨ž?%Îs)4€?ï_<ƯÒ@?™4Ìs2=?"ô&¦—`?™&*b¸?uoÄÝÊ?‹-‹¢Œ½?îcnès¤ñ?³¸<*ªWë?§.¿2?³bX´‰û?—quŠ]?•~èüìQ?ë1eY1ZÒ?«ï"™Ã,?ÀL8¬ˆ£l?ª4ÀÂv‰T>+žìÂjr>8ð÷Öý¡?ïø÷!h?IiÁ£1
?O蹁W?Ii½3ò 4?2o݌ƒ%?2ÊGÁ"e?ï:™c5Pç?¨V½Šë?˜bÍՋbI?|EJs'?iªFí$³?—e+»?î¯þ­Åu–?¹4V2únÀ?£ep·Âr?¸Æ»üõþW?Š\Y˜ÝÙ?Š6a(‡N?줠ZlÍ?§šÀ»:‹ê?·"ßÉPVà?¦VK¼>4¡Öâ×>I*
¸a?ïòûªREê?Z¤
MáÙP?Zª£I1?Z¤ßîYéPSR4FGL J1742.3-3318¿ã¼hÈZ;$¿ûÚà‹ÆrÀ8ÜkÝËùÀ;/:Wꢡ@ŝ7³Ët@tEêPk?Â|˜1º?âú'
‹þ@–¿Ê…Ë?þ=šOw¥¿ê}©Æ˜?
Gç¿×!³ƒûw°¿æhwM>w4¿ímpEã9 ¿ë&€IRPSRPSR2FGL J1742.5-3323PSR J1742-3321?™ í_?šÑ#%N?ìV£"ˆýY?·éè/Š?·¢ôƗÓ?³×rõÐI?œŸ­‰k?¢Ìˆ ¡@o?ã½Ä›Ûï?Ĕ®Ò­ú?Öº"ï3ì?ék¶e
?²¾Åàwä
? 2…×MŒÙ?å4h	~®Ý?³ºÈ§ö+?Ðç~u7ã?±<Ô'd;÷?œ5.W'þ?x¾ü "%?ç*ß?ý,L?¦Ìñü*_.?ÏÍÓwX/?¦¨?×{\ƒÂÏ?{‡˜F€?íF³ëÕPª?­µÚ	æÔ?³q3µ>Z?¬)­3»?…<
ô?GoçTɗ?ä)Ñu±?Êônšpß?×K4—ób?ʽÁoT?£dl«p?'Á˜ÐÁ°?åéÞãÈ?º	Àâ̓ñ?ÑÁn"ö0b?¸6ƒŒuø?yCG[hñX?`"bÛVzN?é)åñOÓ?©8µ³h"5?ʽ>.¹ÑÈ?¨èî,3‰PSR4FGL J1744.0-7618¿ïpñ"_üÀ6t¾ÆyÌuÀ8¦-vZÐ0À<óý">6@˜rÆñìl?ü̲{ï?¨4_>e&²?ã8MžïCð@3Ö}sÉ?ü'@³½?í¸Á>#Q?ÔY3wü'¿ÕfŸÜ©¹¢¿åü­_I<¿ï¡±Ë¿†"¿ïüûÔ!TäPSRPSR3FGL J1744.1-7619PSR J1744-7619?"3¶MÊÝ5?¡úwf$2?ííjI¨s/?¸iÿG¡¿?§€Bús?²oÊ?v.þ?Å–²…z?®Eo‰›aÕ?ím.Ú¼'/?³÷ïÎûj?ªJFøœeO?ª›†÷´	»?'@3ÂEŽ?>z±]A?ìg»ÊQ ?¨Mª´KÃ?¸2érÕ?¦îø?#
ÅÕ?²fþ$.?ï‡áO)¢ª?xÂȇ°Èf?»ué'Î?x¢C‹îÔÀ?}R–T(k?šº€—ß?ï
¯u<ÜÄ?¤@¾‰ƒ›?—UŽ*dRq? Ê"+~N‰?'ÒtR?›*nŠï!?íá?—÷-?°-†»ýcò?¨ƒÌWŒ"?¬›`¤G¬ï?Œç7	ÁÇ?‡£_A'>?í cœKiz?£üs{Ê<)?³_ü;"¶{?¢ñyǚ?Þãx›X>üµúbÔN*?ïnª®¦m?ƒmj`åP?'"c;ÀsÄ?ƒhä']²…PSR4FGL J1744.4-1135¿ãR,þ:Øï@"]·k;¸=À8r¥®À;T¨ŸÆÚE@¾õɛ?@õ\Rç-¡?§G3¾/?䦏ãW@3áœàu÷@蕫"ƒ?ïþ™côÏ¿·üæÅò=¿à-1üÒN¿êꛟƒ=¿ï×ßÖjÛ¿ï÷ß4®]vPSRPSR3FGL J1744.5-1133PSR J1744-1134?iç³w£
?m¶{ôq?ë–ý4@ð?Â]n×4jý?Á<l`(‡?Â牀`§?HÉ枃?•>§r¯¦Ê?îHœ7>í?°dÞvahø?ªéCú …?®ëG»tn?Œy²JD·?‰ª0"q;?ë9¹z"!¹?­d]Úõ#?ÁQ~ëËô?¬@
ªOŠ²?	à® €?Âïtž'?ïb59ü-Á?z£Ïi;ƒ;?"¬h¶õ5|?zœÄWAŠ+?c˜°k-N?bšLôܪ ?ì˜Ùö£W?ºŠÝêG?º£ te?º%G͟½?xŸ&ý?†Ü¤¥.«?îžàI—?¹Mo·v&?¬ãÏ.>
?¹gl˜&?ãø›.ZŒ?}Ä!3€?ë±>¯?°¼#E$'?Àwhjø?°…»êb›>ßDDE®2S>ÜXW7ç?"?ï[î¼?€­©§@À?"š‰Dè?€­¤:TPSR4FGL J1745.5+1017¿îs^V¢y@3>­-ËfÀ9šVÿÁßÀ< W¯ê=÷@VWwá
!?ÿFôæÇIÖ?¹=uai|?àE=V¢¤@ 'ÛçòÃ?ùð:æ?â'!,öX¿ÜX°»t4ۿӍÈhûí¿âä
k"ÌÑ¿ïÉûa4Î>¿ïÿH˒:PSRPSR3FGL J1745.5+1017PSR J1745+1017?‰ò¦¿á›«?Ž—Š§Œ—?ïm¿-?"sDêA‡?u;#goB1?tw¦L&ìu?"2«M÷?§ŽX˜?í²lèûEu?­¯'Ž¿IL?ªŠ˜¤­/?¦¬6tô-@?ô7Ó_?"èØN¾²‹?ìsŸ=·4y?¥,¿žŠ?´ûÂӀ™c?¡Ú€ó?«@0Ԁ—·?ˆŠ€0˜Íb?éAû&?¢Í–ÿ¾ð?ÄÖïPz8?Ÿ·3ÒM;Þ?4:huÔ?dKä™ïî?ïˆåÓj1?†E»
A8?y$¡'k´•?sE•iîB?‰ßN±HIá?'÷âÐ?KŽ?©´[ÈV?§Àžûô§?¥Ç󹿌š?'ºNðÔ?ˆ¥Oâö˜?í`Ö"Щ?? ³ð
~.?°´ÍºæùÒ?Ãÿ×b¾@?€"0Hˊ?t›póÙ?ê*QÀ(?§Qo1±Àç?Ő•Gª?¦±kŒ.çPSR4FGL J1746.8-3239?×öb›3UKÀY1¢9{LÀ7Ãu"*ÐÀ:ïoɼw@M,…šT@o<¥¢¼?°süPH?àÿ»lR8²@0¾ß¤@?÷ ÌäIÁ?ïë)yv
£?è)8Þm߿ݸõ_='S¿æ°ô>«·S¿îw.4Ʊ*¿ëˆª"¼àÆPSRPSR3FGL J1746.8-3240PSR J1746-3239?_\—›í¥Ã?{µhÐv—
?&Ò?µ·Xi2$"?¦"™ÇÀ20?´ðD?€.«üu"?‰35<€—?ëM"«ã?±å‡«Eî–?ÁȌãË
|?±×~¬ñI¶?Šè…~ÉM€?‹¦é€3?ìÀPEEb?¥×kó΃?¶ m&׬»?¤>˜ïè•?B
Ýs"×>÷—Û€¾ˆ?ï^ñ¥™Ø?{h´R
A€?"<Ç}Ž?{f6ˆŒ³?cH[á5<?pHmšÑk?Æõr]?±Öò\?¤OãZvÒ?°ÿ&ÓË»ø?sþ‰!ð`?ÉEEéË	?즸â›Qf?³
ÞËêß
?¹ŠPYqË?²ß±.uY*?€ÑoT'É·?~MüNÖé?í=ý+s?¤è՚el?³õé¥ÆY³?£P»ô×:¶>Ù{Mÿâ<>ÓÁëÂâ?ï}ÉL˜<«?|_­
¡Ûé?E>Ä#‰?|^Œ$«xòPSR4FGL J1747.2-2957?Ù
ŒbÄú¿ë
ßòC~ÛÀ6'Ôº××ÃÀ9½åëoO@ÚÙÇ1@Åûø3ƒ?¤RRá#q?Ø^TùM@0yJ€à@eݶ•?çS¼_í%ˆ¿Ô¼"E$Lf¿äjšêÒq¿è'kí"¿îCƒbu–¿ìùÍ¡^	 PSRPSR3FGL J1747.2-2958PSR J1747-2958?'_³|î4ö?ˆØAq¥¹×?ça­kÕÞf?ÒÖñH­ü?Щ§ŒT]?ÒÖÜ;àõ?v¤È1±â?'}I=û?êbç}ŸŠl?´["ÒïÌb?Å¿;È5Áá?´gùt±¾æ?œÂs6ì@Õ?˜¶6CšØ?çÑñ¶ó?³~îG›Ë?Íê¿Y¥@?²±Yö Ã ?;¾Aâo?Æíß6Û?ë9V×A	?£j÷¿›Š*?ã,ŒÈG?£idúìË?y"7‡Sº?x²¼g'??å
Ք'¿Ÿ?ÍgÆ[b¸?ՀJŘru?Í<1xaÕL?s*$'˜µÏ?€è'7mc?ëXÞ˖±?ºkÕñ¶ø?Ÿa.Ä?º=YŸ%1?–+·}€€?'¤[Iw¤?çÒÉ@{EF?·Ažæ¢›?ÍïdÐÛÙ?¶d0€¹>t>ê7!Òÿ\~>㥖³‡n?ìMe´åÌ?¢ÄgƵFù?½"¨qx¾?¢ÄI,«PSR4FGL J1747.7-4037¿¶Û,™¸Ž¬À¥P"WBÝÀ9"A!"µÀ;ϜÈù¶@,ØCxz»@ŠwTË?´–Õ™úèi?ܘÞ]ÃՂ@"'6¬dwy?ÿü¨G1lß?ïÉ%x_.¿Ûz1¿•¬¥¿ãFÓ#(#¿æ£»-h¿íœ=þ"Ci¿ïüe¬,CUPSRPSR3FGL J1747.6-4037PSR J1747-4036?a¥½àçî?cێŸS6›?ïGÈ慧í?'ôgJ°á?"Ò+‰Û0t?'w¯Z%?"1˜bé­y?›eÇ]‹Ç*?ç©$BÖ?¿ô–n°¦•?Îõ;ê—^?¾ÓÚvó@C?®¢=×üÖ«? i'5=|?ê>3²½Š˜?¬{	¿$ ?¾½C~?é?¦0Cwy?­ÉLX?~¥šw—"?ëWZÛÔã®?*˜¨9?½Ù¶Þ+¢y?œµÅŠ"`R?g}Ø×GÔ?^êk‡¥2Ï?ïõcU )?"ä7{!D?š1˜uχ_?"Ÿ•ƒ ¹?'û"}/äö?ˆõaDÔË?ç…_8R_|?Ån™KýÏ?Ð]h{i'Ð?ÅLå"¦j…?¡Ae1$i?•—x™°?봖Ö×ÎÅ?©F›šÐ¦K?¹Ï("Bª?¥Lnq€É?t÷Ô
w]ö?[¾e´ÅY
?즟¡U?ž([ù?¹{…¶9—¹?îÌÔ%aPSR4FGL J1757.9-2419?㏚µ"Œ¿˜K?™s-À8xh¶¢¾ÜÀ9ø#CÑæè@ 4ÇÞ%²@«¨?ùA7Ì¿a?ɳ‡i!,@S™ V¸@d¡¼'ãõ¿¶ÍgÑöW?í»
bY'l¿çæ a3÷¿ê^˜q{m_¿é*qš!¿Ð1Ácb%PSRPSRPSR J1757-2421?ÇÇ˚?Âȯ;—ZÐ?²2IÕ~O¦?¶nzâg?çóx~u?Æiý·GÌÀ?¼6¤cC"?ÂŶœÎq,?
‰Ô4?¨GËh4'?ëì§2´]?Ã9¯%ihq?ÂÂÅ,D?¬?«EüT?¸Ç>DGþ?¤~q¤Kèû?è6l
Ù½?°ÑjüE?¹è\†yè`?¨¶Úƚ?wótâA1…?‰Þ½…Êf?ì"
…=…á?¨>‡1?¸´S°ár?´HnÉÃJF?°‹~ßë×?µêTÁ$,?êî9™~Á§?À ŒÒá¹Ä?¹"P{ÙÅ?À·#߇'?¤Ð³ÈU*?µ'¦ãšt?뒢Y†¯?ÁÖ…?Íÿ?¸æà>©}?¥ è\9*³?½g¥çÁÖá?§ðVÇenj?é62Ï`%?±¥Wÿ ?«eNO£"5?²©
4ÆÜ?Qr6Ý¶S?ˆdÐ¥y•¦?î@ñÿ®˜Ò?³
¼w²A›OTHER4FGL J1801.2-2450?áŒõ±Èdˆ¿íÔPXÝèÀ82ÿݛQ*À:šÂn¤ù@=öÔ{@B­Yiþ¡?µÚÎ~cïO?ÎÄ»Ü9§A@>¢Òþ??õåC¼s?íÈDÝ¢x¿ßÆ:ÂÇ;¿áõDD¿ä¿T_™¿é…¡—û¿ïÿ&PÌ¡.PSRPSRPSR J1801-2451?¨w]ãŒ)?£yQæ×®á?ãÕÁVæ°h?ɸ<ᡊ?ÕE'±»ë?Ǎâ¹xæ?¡o7s'?¤`0H?ݾÓp¼ù?ĚÍÐq¶À?à	>®€J?ÃêvÁ—(?À+¶k{<ü?¤¼]ÔF"¸?Ø0ôdÌ*?¶,Päöš?ß¹0ÉݕX?¶,è¹üáI?Ç×rd™?nš<¶-;?ÞdžŒv›h?§."°· ô?à›	'?§26é3%j?—yÌcŠ,Ù?'"ù"C-?åçì¹ãLQ?Æpár(ð?Ò¸‰ÆŠ4ï?ÄüŠCŠ?"¸
äX±Q?ŠœùÕ¬_é?á,Ue®?ɤ§‰ò1¶?Ý!æþû?ÉQ.µŽÜk?²<9"R¾¨?ŸHç(v¯?ے(~Ún?½hÓ,|#¬?ßÞÉ:,\æ?»gøÑ|MÈ?mU>ùû…?S² '/ S?á»q»â¢U?°Q…oˆQ‡?ÜNrY8Ö`?°@9_íÝ[MIXED4FGL J1801.6-1418¿ÖðW'Ñw¤@Äk¬÷DpÀ9ß%"åÀ;ÕWµÉ{@Ə§þ6Q@3ƒB??±?Лl¢À‰È?ä›@ãŸø@kf¶~¢@_s"\³?íYiþ¡[/¿¾ò\=îx¿ê5ŽøU瓿î],áŠt
¿»ÂÚô¿ïÿðÇô PSRpsrPSR J1801-1417?ܤß&°\Ã?Êv+Ô!ÞU?¹%ÁŸ`ò£?´J2?	®"?Ý°qwf"?Ʉd¤ÖtÒ?àj,*?ÇÀŒÍƒV?³ 3Մ&L?²‰'·Í-½?Úøó铤Z?ÄÚéù‹û?ނ÷_ûò?¶¬ª(Ä*£?ºì™WÂ|?¥·phI ?Ú½²Üo?µ£÷ô‰Ms?Ôú"Ä('?±þù$+Ÿ?³ÙRo£ ã?¢éü]‰?ã"OÜð?±qšìOÕó?Ó>ø‹u?Äp2Ô#ê?ÅíŸS•O?À
¬É«?àùù)»Ôò?ÆC¼ÒG¤É?ÉÙoÁó™¯?ļ‹ó1e?Ç&!»N¹?Æ-R¸<P?ãÀ ¼Åæ?ÆbüŠ»Ás?ÓʒéYÓä?²XþT‰c#?Á­v8t^?®!Èe×B?á¯Xý6ö?¶a6Cyu?·e'Çh?¡dï))UJ?À-'ñp?µ\°ŒÌÃ?éNŸ±qä?µN¶ª5ËMIXED4FGL J1802.8-4719?ïÿîÀ^øÀ(qûÅޜÀ:šÉÓIÀ<2w¬ßÇ{@ÃßóE1@@˜ü»§á?Оˆ@Ö´Ø?â9Ž—@§ôÛߏG@؟ÎçÚ?ïy ÕÍýN?ϳù—02οâ¡sîeô¿éÅ# ™5¿íŽÁ.32¿ïþ"ÐÜýPSRpsrPSR J1802-47?çwøt5:?Ê]òCÔÁ
?»ÇDvt?¿@'¤)añ?Ä<œÀŒïß?ÃSå7@£?㬽X¶?Ê&nXø??ÁÀ~úuÁ<?¿@"ˆ‡?ό‹¥Kd¿?Å|'Ι'?èrƒ¯ï¾·?°Tx×Þ÷è?»^áå|‹?¥¿Ã¢ìy?À†íQt]?¨:‰u¬vã?ãp'j˜D?§Î"å9P?Ñïe¨ü8?¥¡'°sA?ÀیO¦~?¥3è,'9ü?ã,ðà°ã?ËK=‰+
?ÅɑÑE¤Ç?ÀÏñÿP?͆k7—­?ÅöŠªÏˆ?Ø[`R?á?Ì[
"!Â?ÒÝ*›' µ?ɖ·ý\â"?ÔÇu.^k?Éu:îØ);?ãC4V/ß?¶ÎÆüC×?ÈVYþÎý?±ã ¼«?ʜԨt?¯	îÁ?Ï÷Õ=xuK?©—÷éx?á"æHÁ1?¶hHïÞ?ÌÛ)d…ï?´AaùÌMIXED4FGL J1803.1-2148¿Òzª©iùÌ?Éx.û@'¸À7"èG|–TÀ:´v"±Ó@çûZ(ë\@µô^N?¦X"Ãs³?ÑÑ	\õúC@%DæŠ
5@½í;WD
?ì­nB}Óë?îè* dú¿à;­àÎaw¿ãˆP›ùÆ*¿ë˜K$Á€¿ëõe<š»PSRPSR3FGL J1803.1-2147PSR J1803-2149?h'd×Õh?qQiÉW*i?íÝ_H(Òv?®®Ìµò?°Pr˜<¼
?®XiÐ2šÍ?zN
M?'Ð÷Ï!?è&«Ä-?»]ÏWÛM?Εxh­¤¥?»o"øËr?¡$úë?—²âqtÚ?çE…"J
?µ(E.?ێ!j?³Lý÷?]È2æ¡è?DþAî+?ç™!«‡û?©ÖF2¿Dú?ЯõÁb¶Y?©Å…j>‹w?[Í¢Þ-q¤?Sܶ	ô‡?í`¯+7ww?®¦—¥h?´‹Pú¦E?®]EÏnÇò?rÆ
ô?ÕU'Ç®?èJÁÏe$ê?Ã×ÍDIŽ?Î>ÈTd}¥?ÃÏ
#݈?‡ž_ö•?#è›B?éé ,Æ1¨?²±(mN»d?Æcfyå'?±Úµ@œ°Ù?6šëã½q4?&`·#ù"?é/—[?¯Qv`Ì¡î?Ë6V†Òö?¯Kµ PSR4FGL J1803.2+1402¿ì%!†@)@0êkƒÙ^À:˜û܄еÀ<[›]@@Ìxé÷@Ò¶»éOº?Çâ·ðœ¶?ۘjû .@Eâb`Gh?ö±Ûø8áH¿àfç?¿³Š?tÈT0󁱿á¼v¾MX#¿äHb°Ï@¿ï²äXڌ©?ã÷äþqàmPSRpsrPSR J1803+1358?áË×]/Â!?Ä "N"f¡?À>òÀ7¤B?µyÃãG¢&?ÔH×äqÈß?ÁÂ8˜¼"³?â¶Pê(RZ?Ë
óÈ}÷k?Ò¨jŒÿ?Çäѝ¹[M?¿«Ð06?µ"È5¤¬¼?áÇ¢íïöâ?³¼&Ç ?ÌÄÌD´z?®Å³btg§?̨Œý?¬z>‡®h?â‰É©'?©›.Ð:$?Í #<KÖ?¥ÔPŠîZ?È;¤ÀX#? BðÃ¸×?ÖÙét'?º¥fñš?ǡԑ_Ï?»Ó*A?ÝU,Bå>?ÄáC*»Ú%?ғ$
à?Ë°ü
ú`ü?áw¢îF?ÏøôŽîÖô?ÄýÁa^¿©?½¦% ?ÙN6âÈÀ+?µHæð+Ïü?ÔQ•ÑZrŠ?´Vg/ðû¯?Ò`3KÜÍK?³QÃäÖ4Ô?Ïâà,…ù?¨g™—@Mù?Ú Z˜/•?²ÞÂí2Åe?Õîxdn-?¯ƒ¿ŸŠåMIXED4FGL J1805.6+0615¿ÖÂÓº&×Û@*΅3±À9öÝpˆÿÀ<1#|
Ü@Þ~Û¨1ã@"à¤ðæ?Áw'iP{˜?à"<›<@#VSÉ«°@ßT¼oÝ^?ïâp"&ñ[?ÀÏÅ0¡¿Óª;½ÆI¦¿à눯fŠy¿ïÿ©-‹S†¿í£?O¦†PSRPSR3FGL J1805.9+0614PSR J1805+0615?¾_ò.+?ºÁÌ=°º?ëO®a…^­?¾j³
o:‡?œŠk½äÄ?˜kWj^¾]?¶àÃmHDø?´t؝è5?é@•ìæÈ¡?Àu^ä'?¿+ïi|?¸š	«®Ï?ÁúHAH†?¨N´OÇ?è"ò)—m?°%b\ûà_?½kÞ0³?¤võæÝ«S?ÓÁÝ%ñ'e?£5V"3:q?à‡Œ±~½ ?¨lï*eqX?Æ^î!äµ?œ3nœ‰Æº?¢.»tÍå?¢?¦_Úîê?î¾ã¼9?¨ø -e–?›žñ@vG?•åG¼V?¦\'Ȳv?©Ú'ƒp›?ê2Ké?À¹ì­4M‡?À4'ÜœV@?¼‹3(»#ò?¬#X:LÙ­?œJíÓÇV°?ë×­h?¬~^¦d¿Y?¹›c¹±ê?¤ÀˆÖ.ɍ?½ŠwEdl?œž˜¼7?åIҙÀZù?°kÞpDRï?Ìð][áä?§Îù{@8
PSR4FGL J1807.1+2822¿Ëú†'vç@5‡,ƒì‰+À:£àyQûÀ<2È b@4÷â¥&@á'©?͵ûåi%Þ?Ê®¢jM¦§?ú†¦\ö{?ó™–dïï?âqíþ ¯c?íØ涂޿é8h\	ì¿ë(0Àè#¿Ç°I‰`çK¿ïÿb¶®}VPSRpsrPSR J1806+2819?ïPR¨ÄYâ?'™A»ÿM'?d¬Õ¥ªDE?d½4;	ƒ?"`9r¸:?'Tc²ìvÂ?î:Po?¯YÿßJˆ!?— R/¯*? ™†Ÿýòñ?¤³A²é&?¤ûóÚA?íÈ«kV[?œ"VóýtR?Ž]¼[«ñb?‰Ü´•V:‹?«ÝÚ1×k÷?˜ž".Aö‰?ìMd6WÍ?šk)ÅÆË?£`ŒD·ä	?'¥"A{þÝ?³æν©?úf·9՞?î&n'?¥¹ŠdmHö?|Xµ"=;¢?~åN®x˱?ª)㬢?¤…X"ŽœÒ?묦ÍÅ×?ÁF%J´¦ˆ?°Y5ÎF‰!?¶…¨P4¯?·™dù"z'?¶—5€?ëd¥QfW«?§Ê€Õd?Ûåä"?'ݹhÌz?½d{Â2?¥KÊi$š?æ><£Òá?²8^=•?¹c®ŸúØ?°ëÁ&í?ÊVÇE¤O?§øˆöëAGN4FGL J1809.8-2332?ܖeâÝÛ=¿ÿóÔ
2îjÀ5˜µnvÀ9²æ[L@ÔQÞÄñâ@ܕà•×?½ÅüV±?ÕÕØ#ÂýÁ@F-¯ ê[S@''[²ƒJ?ç´4ºò¯µ¿Ïñ¤ƒ³ÿ¿àÞ°z¿äé^¾Q^í¿ì¶óé	¿íI³bmˆoPSRPSR3FGL J1809.8-2332PSR J1809-2332?) Vcॺ?#мâªù?î£7œ=Q´?£PœäGÖ?¥²åâEЇ?£K%fm§‹?o(8
¹é…?ÀñL]üŠ?î7ï<…¹µ?±ÑÁF˜B?ªŽˆµÄé?±_ÐÉ¿MÊ?uõï¹iv?}Àm¦"?îû?¢«‰V—'?¬mQÆÌÕ?¢ ¡§ƒ\Ù>óÚNxh>\P{ºf:?ïâpncF2?o'½ÿáÁ?m'	ª‡(?o'3/ª'?6åA5ڇþ?1›cÈó`Å?îÔ'`9s?¡!†çª?¢ýT.Iw?¡SôTîG?_ÿç[R?uøŠ˃9?îÅÎ'¸"=?²zèÆ«à?¢ª]'¯JÅ?±îßœ/v?k»#c#¿7?mÓmd*K¬?î[~ª;8¡?žÛ©"TUE?¨Œc)‰Õñ?ž(̧ãß8=àÉÖÑaµ}=ÿÉÑ)ù€n?ïÇÛ§ñ?'?9ýUï^?|uŒjÐ7?'?9öέgPSR4FGL J1810.5+1744?éCr2Í\À@0ÏîÑížÀ8(Àéi¼À;›I²Ñy@fúÅX8@Øu'ST;?§L&Ÿ& {?҆µ¼:…@%p÷…@ÖoºÜµ?ì÷ì5Gài¿Üd…üðJ¿ãÌ©C6Œ¿èä"ŸR¹¿ìô#ˆ›D•¿ïó!3FPSRPSR3FGL J1810.5+1743PSR J1810+1744?"´õÃû'¿?'Âh$>"3?ìîs*š~?°Ï³gå?³_)8çå?¬BðîÔ¯P?šê{ÏÓ>5?œáݚM¿?ìÓǚUM²?¯`TvÌP€?²§$;†"b?«äè0õN?ÅqúgÔih?­,õóµåm?æQy—"9?²v'ôÁ§c?ÁH9½L7?ªìô_Ú?°Ý¬$uP?"•ÝpŠ¶æ?鳦Œµõ4? –{>%.Ø?ÀÂáu•K?šnÆ/šd?Š±®«}Š?ƒ=|…ÿ·?íY_9ÌT'?­4͏…èŽ?±ÞÐZãàÁ?ªº²Y^4!?"Ñf±Ý)´?¤³:û5?íMé!þ?¸ŠovÂ?°_-¼?¥¡?³ÚŽ"/¼?²ŸT¡³g£?£6ã™#?ég~¹Þf?±Y¶ª¡~À?Á]TØÖ?¬[§ÿ4"a?''zàt^?zE'.ø¾?ëèÍçÝ}?¢>>8¦¸Ý?Ágml¿ñÈ?¡5¿~«b·PSR4FGL J1811.3-2403?åÚ¯T}ÀWg?ª9ûÀ8µml%QÀ:'
©§-×@ ?z¿8å@{Ú¡¡¥Ø?Âü$©,µ?DZéDŽc|@±B³÷+?ínÀ	šÞh¿îÌÂn¤ù?êðL-Õü ¿àÞ	|¿æ°¸.°´¿è‹X=®·8¿êGM1:ÇPSRPSRPSR J1811-2405?Òÿ–\½	$?ǝ`Ȭ?Æ"¼'Âæ?ÎßSÞµ"±?àû¡óZU?Ìð<ÈIŽ?ÀOà—HË:?»æp%ƧÞ?Éñ[`º?¿žE6&=è?å«Kƒiµ?ÀâÖ4»¯ª?ƽڵŸ?«x¿Ø"A ?Æ=¥/­uL?¯rÅ\z†,?äï'=5E?³C^s¼Ê?£[ë­|n?ê­V''u?ÈɛIÇõ"?£B5Ý!ÿ?è—Úsѐ?¤õo£éä?Á˜ö¬<?¾)zë·&P?Ôwnη*?ÓÛÔ…<.?á^oZù\?Ñv×Áâ&ë?¤šÜÓø?¨F5÷ç5a?Éΐöv®!?ŌÊSJÕ¼?èLT‡8?Ųg_¤o$?»vVMj'?¢åÍlÁ3?Äûg]Z?°&Ey†Ô›?çR[e''%?²Ó,)ŸN?‰j/O¢g?pPVò…î?Ë5e'©?¬iŽ/ Z?èÍ©×̨?¬«1¾b)OTHER4FGL J1811.5-1925?È$Pj¿×$2#é".À96"4ÕËÀ:z&­é²·@!Ë仯@"Á¨¬\?âA{_ò®ß?áL!¬"2Z@«ã	O4@Aý#,?ç…"~°	¿ïB-¡ú?î•TûÚ×R?ä˜Wz:¿ä…"ÿ‰b•¿êî~F¬ãPSRpsr3FGL J1811.3-1927cPSR J1811-1925?¿"‡ikS‹?·ïj‹Ò?}ËôG«‰?OŽÛ°?ëá…z—˜?¸u "áXQ?ÏYàÜƌ?Ï5´ a?ŽdÚÕa'?˜ç;C².?ç°+\WÍO?Îà2"oŸ(?ÐË0æí?°ÉiÍ ž?¹ÝòŠ²²+?¤bå'4ˆW?ä^© š6D?²z"‰V{?½ÐVjÖôª?°Ø¦@Ñ>g?zíáA¾YI?ul2®Øý?ìp>p?±½
Þ#Ž?´y­p/Ð?°¼‡Xš
?qX':G?näÔ)‡=Å?íN™?± Œ9)?ÅØ	èOú?ÇGƆ?RY?‰	éuÀož?£¥Œlåz{?ê%ÕW"mc?ǧJýTT?ÉfÊ ˆÝE?«BQüO…õ?¸»Á.*',?£Ù¸l¾PO?æŽÕ2xi?¯ýìõ@+?«uÅ«Þ?ªœoÛÜ¿q?rlNOËÈ?€9 .?î"Ö|è£?¬°"ÎVú3OTHER4FGL J1813.4-1246¿¡Ãã9Îú@Š.ÝcÀ6×1ªœ÷À:O"}Š@öÃì(ˆ@?_[°)ÿ?'D$z¼<d?Ôª±ïÑ´"@<ÜÇÀôQv?úû]ƒé¯?Øhà¿Ô¿Úâ'[â©Ù¿ä²)³W°Á¿èѵ¿¿óö¿î2ò yI¿ïþ Eð¥PSRPSR3FGL J1813.4-1246PSR J1813-1246?E‡ÆÈMÏ}?K&o˜g!‰?èxj!(f?՛¶n*nØ?ÎÏ´€<?՞êiž\Õ?i^V×cï?{·T|%?í(\œ|ç¡?·wK˜E5Þ?µò(dUȒ?·Nãtá*?šÁO‡Ç?–+
}t¨|?çùSM¯á/?²ú%fëI?̏ß(?²•œ{Ú'>–{ÆÕûÞ>™æÒT³[?ïz_Ýé³@?"S"4?³í¯z¿T?"î*[Æj?MwŠâTÚ?ND½uX¼?èrâY{ò?Ñø°;­¼?δŸ7?Ñœ1é ?aêŠòê2?rà¢]á?í±àkvVÛ?¸VëÒª?±á¨M9åA?¸¢¼‹•?–î؂þ?'N6T®P?æ-+ԑŠ?ºdU¿û?ђ¸Qæ
?¹c@[Ù¨O>knp£Éà>{hºÀ¤?ï[ñL«KÀ?‹S˾‹¿²?"Ò÷ŠðÇ?‹SȝöÈ	PSR4FGL J1814.4+3132¿Ú8œNT̶@5²køvŸÀ:LsGyBÀ<&_ċµ«@iº-ã¾@÷òeÊ?ĬÂkIû?àW.ºþn0@±¬Þü+@†Ð.C¿ìw6b'œO?Ԁ÷Áíö"¿á³p:$¾ü¿ãˆáá¿îÞ>s³¿ïòýƒMýºPSRpsrPSR J1814+31?¶%]?³ÓP"ƒíÉ?ì™Q'îd?ºx¦'Ç	·?¡þ<£¢Æ?¢›úù¯#²?Ãց
~G?À…²m6J{?èI½H?Äy›stc?¶
÷üa¡?²!wù˜?È|"õ‰É1?¬B4~ûå?åo™} ó?±€.ܳàó?ÁÅòYñ…?¥1‹pêq?ʈzãK?¡&ò4ʾÔ?ãiTœÎ"?­B8vÎoc?È?«mâg?ªÒÌªÖ?™¯ðaì?"ë°Þ[?î9ÙxŠ]ð?¨Á¨g£ä?Ÿà"1þ?¡¢°.0"ó?«/[¡7Œ?°äBåK×k?ëÖ/ gÐ/?¼\óò'¾•?³¶Õ+ÐoB?°ÇØÈà?»d?"]V?¤žTV}ìé?è< +2w?°Ú–œ¶šá?ÁGÍ3¤ó?§/Ym†Jš?§}Cå—zÚ?‰¥ÓëxT=?è3PtŒ™×?°Éyų?ÉSm3ùÆo?°Ê+O PSR4FGL J1816.5+4510¿êò©g0Õ@8¼`ˆÖÔÀ9O¢ÓÔþÊÀ<Hm'ÓÒ{@e}x£U?ý¤y&\‹?°!ñâî¢?ØOŽÞ§«@$­1ã§Û?û˜'©í?åÞo÷ß ¿ÑUU|´0Ÿ¿ÖXZ_=¿åW¤A=b¿ëße‹u¨¿éRlžä²PSRPSR3FGL J1816.5+4512PSR J1816+4510?£ˆÎÝÚ?ž¶£ë'?ìÇíÓ5OK?³2"$Ã6?¯ø"Moâv?«ÙÐJÎ.?RÃ?‡Û?" •óX
?îE(þüË?¨¬æäŒBT?§rKÒàcã?¤¶PÎ=?©È3¸x³Ä?òö°Šœ³?é$+V×
?±¡a™_þf?ÄýEµÈÖ?®üëm^é?«L&"ý?'oËÁ"Gf?êâ¸N†Ë?¡ƒkg©Î?»Cý	Df%?š6ˆÏ³6B?¡Þ€]ÆJK?š0ŸuŸÁ?ì\{®¢g?´W™œñ(Q?´,â\7Ÿ?¯`—×cù?ˆI5sÂSÿ?k4¯É­?îfPY3Íã?¤Wà}'?£ˆ­bðØ? ´a_B:?[‡D•L?"(¾²±,?êÉŽ|Ú?¯ÊÂì°4>?Á8Uñ'ï?¬9ܪgÁ?'X4UW
?}" £zú5?ëm<9Aj?£DØ|Ld"?À 		éã´?¡Ãç"%ðPSR4FGL J1817.1-1742?æòI0ÿ
¿æ¢1ƒ/ÊÉÀ8Xw…À:žé|/üG@侊ê™@^¯ûÛ®?¹¢e^î;Ì?ÚL®ÁI@Åðáy?ùžv*úÕ?ïzÙâ)U¿Þ×q@ŠØ¿ÞƾÀł¿æe}'%¿é™ ºö
´¿ïÿý`éNäPSRPSR3FGL J1817.2-1739PSR J1817-1742?¡+¨ù~ž¦?œ3¾íg×=?æ8mÏ]Ã!?Å¢ôNhe?Ñi¯Aݬ)?ij{e?£ §¸'Äm?¡òýÏSXÐ?Úþ.cµ?Â!yj'³W?áNÞzÒ·¦?Án§-'?³ù"'OçN? Õ×õ`D?ß°B¨Ð?¶íؑNY?ÛÿëéÇ|?¶'¸"|;t?"·A
¼e"?oHˆšñÅï?ÛT½EŠ«?¥¶8T"K?á¯çTɗ?¥Å
]-$?"ÉUÿ"ûÒ?'ÁóŠ8Ä?èþŠš«Åõ?ÃPfT¼?ɌªÕ£'s?ÂW!^
k<?Šã6øbóW?'?û÷ŏ?݃Æ,¹`M?Ç=Hì?àҐ
Ý@ì?ÆÔ*Rþ™g?©qª6PÈ:?™–,vŽN?àó'—7ƒ?¿4ʞ/'¤?ÚêÌjYî'?½œtTæŒ<?s{_ٙ¹?U«ô™©6«?ß캰³‰?­N!R?ßÆËþ"ß?­/â	¹«øMIXED4FGL J1823.5-3020¿î43ÝÀŒˆ¤~ÏêÀ8üŽ~³dFÀ;ðåÍNÒÌ@H"Î;G@4²ú"¯u?­‡€sw?ÒãÚzµRÞ@ C­Ò^Ý?îŸ)º_¯?ؽa4"¿ÙØWdÀÉß¿à8lXï¿ßÓ~—µ"Ë¿íÔ§¢òu¿â#ÎÜq…~PSRPSR3FGL J1823.7-3019PSR J1823-3021A?'¦œ£ØÃ?œ8ßVÜ?ï
y|\‹¶?¤¹ujÛÙ?"ýÉ&̈ß?–âå°!,?"@Pe
Äæ?š9¯µK)?ç|ýcy[?Á7VvŒ×È?Ϥg{[¸?À½Š‹DþH?»œ2>Â?§#$ç"àì?çnKÚkh?±áå,9ûÂ?Æ'øN}2þ?«Âߚ!,_?˜*PÝÿTR?zò¯z?ëUIX8¦:?¡ª?T	ß«?¿K!Ӝ? o—LR?"ÚÒ4˜?¬GÅJÿ+?îLP›×j?°«M7¬†?¦3'ä!0?¡ÌãÚÆÍ?…u>ÎûXÚ?6<F+?ç¯ö~]9R?Æ÷pð1?ÏèÒ›e)?ÆÖ¸52‰7?©ªÿõ""E?š`ÃÓMæ?é¼4€)÷?®‰Ákaü3?¤n€Ò'?¬#e'2A=?uæò
á+Š?a=²ƒ8š?ì3
¢;9ù?£Û0£òõ?½	#Í%?£‰†ººh¬PSR4FGL J1824.1+1013?ÊÖ\'k@%NÉ:qÀ9»Œƒ"_À<tЌu@Hkԏ@c—>?½ø^öÛi?Ö"›Á,Î@ýKÁŸr!?úT"úP=°¿äª|`"Õm¿Ú_3Â$RE¿Ü8×¢hË¿áîg`¿î*= ÿ:¿ïþÃNžÊPSRPSR3FGL J1824.0+1017PSR J1824+1014?Äÿ'€å\?µ9{'Nߝ?äÎ/™(c)?ÂÆ*ÉNµg?ÇǯyÜ?¹MtŽ›"m?À±­•,«?¼
FÃ"?æŽSÝD5±?ÃÑP4uÓl?ÅõÂ~.?¿yèÓb`?Á·A†nTÙ?¨qg%S?åÙÒ÷´,?³% ß,L™?Æár˜›9N?­ŠïSQº?צ0Ïp?¤+\ö·=*?×)&lÖ?¨b˜
"^?ÑÏ3ˆ²Zu?¢€ÄÝ%p¹?´z'=7—<?¦žÂCR?ç.±-VqÉ?Àã¡^£¾%?É'¬Afþ?ºË\Ÿh;?«ŸIšU4?­kMYoÍ?芿î÷?ÅE£vëA?ÆðÀ)®Ù?ÃwS±ál ?²¸®vBB?¢~MA_~?腴Ð+Ñë?³´¹hhŠˆ?ČՄ	4?¬Â뵉?Ãïgp@s§? \	-_»?Ýç'í #?²¯Ô*7º?Ø!Kµò&	?¯	XiAxPSR4FGL J1824.6-2452?§sÏÙbÀfÕ °åÀ81Må"À;6ÕÓËò@ùmqÈoE@=">5ŵ?¬Í`né?Ößf'¥"@$\_|gZ@Ø¢' *?ìå€UÐÂ?Ëoä¿\̵¿ãN'¯rHó¿å*lO´s:¿î™l¸þæ¿×·b|×ÂPSRPSR3FGL J1824.6-2451PSR J1824-2452A?l¶ËÐðÀ>?h Ð},
Ö?ë­á@»ö«?´ÙøÕûZæ?À՟ÍBñö?´†,äSjû?"x­jû¯5?›ã›sÍýÛ?çia?W{3?¿óµ?ÏËeTÔ©Ì?¾E7Ø•%? !¼Ä:-Ù?"Ô˜Àx"?ëä5®?¬H®ã‹]Ê?¿¶z;ä!?©›Ú #_?›?ð'g?~K‰'à?ç¶*N树?¢ù¨1"Ê?ÍÅT[T˜?¡Q=ÁHãˆ?uqt£O™?l§ð_Ô?ì°…H)?²¡Ñ:̂ñ?¾Khé?²*ƒö#›?"ºõÉÃ?‡«¶ñ|B?è_«
ҎO?ÃWƒ¹LV?ÍA8&—1?Â×OèJ¬¢?':K·Uř?‹ª•o‡Z#?ëÔä~¢ÐØ?¬+Tø—æB?¼ÊIÊ-X?ªA9߉bÌ?w,Sª%ö?^ðx¹}LJ?é0ÑäS?¥êÿvnüu?ÊúÆiJ5G?¥³ ½àÓPSR4FGL J1826.1-1256?î¢`_'5¿ØžžôÀ5°¦#뗓À9:FÖ~&w@Šp8ø,@Ú j™Ò?•4Ú¼P?ەn¼¡0'@@ÉrGE8ï@ùF'¤?ïþ"ÀC§u¿Êzأŗy¿àüDôü–¿¿æ"x'Èœ¼¿íøMïwÀ¿ïÿÿ&¦³PSRPSR3FGL J1826.1-1256PSR J1826-1256?Q%'}ü?$ø‹V/Ä?îà—c£,Y?±f85~ü…?¡m]>‰"Š?±³°'OŒ?jBv' QA?z_…Íè`?íÄËwžXV?³ëfX1?±êA?²­ }y?ˆvǐ*¦?Ñz¿5uÞ?ë=73{‹?¯"€=«?Áƒ¶¹*À?®EN
FwU>OC	8o}>[xݒsW³?ïm¹W5W?ˆþƌD?'NÓf¢?ˆå•Ë?¢Ø	òÁ)á?ÆD†«	—?ì»_/̇"?É>rækH<?°¹ˆ©!ñ?¼ˆŒ<Je?`à"!¯?w'àڕE?ÿ"?±‡ð©?¥pE7l¨Ë?±Z>žx?wŸ½êðšû?L>&i;Ò?ëÉSÛkÃj?®)—5Á?À²¡&c?­éÅþgԚ>ê`ô@R>8è}KÓ?ò?ïL™Ïc?'™Òh[ø¾?–|†ú_Ì?'™ÒIo|éPSR4FGL J1827.4-1445¿Ç
óŒîÕ$¿ø<äŒ×êÀ8cã\[J©À;+ÞUõÖ@Y\·Ý@m²¥Ú¼?¿K¸ÿÕ&§?ïÿójÆGx@#ØÛÎÈO@udǪϿâMš¢®R?ï9žÝ%`¿Ê²wa
†í¿ãÝek"£'¿ïùãñ¬€&¿ïþ䬽bÌPSRPSR3FGL J1827.3-1446PSR J1827-1446?KtLI‹ÂO?PTæ0&Ÿ?ï°!¨Ç4?…Þ·^?'@PÿT:?ƒÆmÌܜ?êY
ïXy?ŠeÊ/»@?êÜ8X>¹?µ¥x¬npg?ƅéŒS¾w?µ Å
vò6?"90Î)R?ŽX£~K"¼?넧sï2u?§	—š›4??¾Ìx,ü&E?¥}'$Džq?G*~q
}Ü?1Ɍ㦳8?îÎÜâ{`?‹NËcAù?¢µ"ú]¼?‹%¤´'´Ç?Pû_]H?R—(Ü?ï·éÔxw?"^Ù<7aî?ÌT®Y‹?ƒ?Ûµbjá?sïy%U?*"¼Ž(\?ëVþô‰¡¡?¹ô·a&?ˆcCú´?¹húr'è§?ˆM-DÁä?ƒÝ
âð¾?쎀¥›Ÿ?§Àh҆²þ?¼±æRÀþI?¦pH|†A?2EãúðÝ?iM¶Ò®+?ïGÜˆ<á?‹Z'ØK?–ö/FXn?‹Û˜×?PSR4FGL J1827.6-0849¿íÁ©œWJP?ótx]ï"À8E`؇ëòÀ:¶6eÃ@s¶0(@¼>	P?´A? ¸m€?ǸTÝ¡±@ÿ¿ž ß?óôÃ¿ÒçƒÝD¿?ïðÏ@D"®¿ä¶ÉöX·Q¿ä±F^‰"¿ë:¢hJA¿æ"ÌàîÂÁPSRPSR3FGL J1827.6-0846PSR J1827-0849?¤'pΝ}?Ÿ2g¥9?Ìí"wú¡?Ãí`§EåÏ?ç'@U@àV?āâ@¯ü?í‰RFZ? tÍ?5
~?Ýß»ô¯·5?Dz
FÞi`?àˆµ»Z«ê?ǖåêÕ÷C?ÄkÜcT¹?©¾Óvö[°?Țà5à6·?¬µ&1Õօ?ä¾Pî/$?±ßÆ+ve?£ÙÄè2öü?~î¶Ñ•¸Ô?Üc¯nå]_?ªºd—?à‹ùücq?ªù¼Ø?™.¸íJZg?ŽçðX?ÐÓ÷®¢À4?ÂÜUZ>S½?æ̎`ÖY"?Ã&ÊôIWQ?"]7Åñ<?–M¨?ÔË,?Ýs"ƛl?̏ð+)W?àôúª\µ?̑ïÁ™gð?ºe¸°–`?¢¥µ›R¸Q?Ê]";ƒ?±Ö×è÷µ5?æwQβ?³}j 8°?ˆ:,»c³?m¼:†X[?à#\cá¯f?³@@0‰?Þøug`6w?³cGàÚÄßMIXED4FGL J1828.4-1059¿½œ¡izJ§?£1]<F,À7¯<Kà©#À9½Ñˆô/è@^Ä[@¸•";"+?½¡§Z!‰"?Å¡… eÑ@
2†!î?û§)Æwô¿ÜW'còà¿ÍÇNފd¿è.®è¿è‡B_ ¿ìŠ)º
­h¿â–¹‰$PSRPSRPSR J1828-1101?ºŠ¥Ø8³?¸sw}"?¬c"¯!¢?²9UûÎܶ?êèsLäñB?ÁjÉ2ʓÉ?›šoy×Ôµ?¢Š"7òã÷?È9ä·>	?¹ÚW­n–>?é³Va¿?ºÚ… –'?µ\;½ùÓÊ?¢ì¨ÖÀ™ø?»Ç⤜ÏQ?¤¿É$Ê?éÛ|3ñãÌ?«)5LuÌ?"èCZN©Q?sm¸þ?¾¡Øº8B?šOÅ_ý?댂ÍØÄ?›Ê¥acî?¡^ÛÍX©^?šyC·¦'?±Þ[@·Q?±úšUû?ì®FÛa ?´Kru¤ƒ?Œ Yv0ð?«Þ+/Ï?Ì®ÃÍIÊ?Âõ27›ß?èˆÒèÖÔÊ?Âv0…ü%?³ïZßR>? Þê¿N?¾íÍñD?ªBÊ!n1-?é¤[זT?¯¼`záj
?t>³J–æZ?_©˜¹£ð?ėûT»,?¦ÐÿÏh…?걃ā_ø?¦øÀGb¨OTHER4FGL J1831.5-0935¿ï¡ü"¿Œa?‰"ÏväýŠÀ7íèPïÝÀ9אíùm@Œú#G,å@@E]b×?ïd²Â4˜c?ÔEµV¬µ?ñÕ9eQh}?î%eJ´O¿Ëç‡Ù¿å4µê28¿îx8@8TZ¿ï|ŸB¥ìä¿ï÷8EÁ«1PSRPSRPSR J1831-0952?Ãa(ypÚ3?Éw^ü«?—ᄈÉh?»0"8ßù?êh©½†¼P?ËëhTŽ]â?½Œeéé¾?É<Yç@Û?Æøºµâ¿A?Ë)ñmß?æD•Jl?ÐbDhå?ÄÉÐÝÂWB?©VˆÃׇ?Á•Q3àh?©ˆUš(o<?æhJtBr?°uìo˜?"ÞÝ]K/?‡«Éœó ?åâxa èi?Ðv«NÍÃ?ӚPFGÅ?Ð,ā,n?¾IèE=Å?ÅϪØ[KU?¹:¢'®?­áÿñJ,?ë°ù"êª?Æí¿-?«UXøÄÁH?¾aØsZPë?ОÛ@
º¢?ÒsPH†›?åû<Ð|?Ò«™:=?ÃM1Ê[?©b+ça?Ác7ŽGè?ªRá8›?æÓåª`³–?±~ý¹ ??Yõ}Ø4jY?dFÓ¥	^€?à×,)?Ùf.‹aP0?ßÉðÓ«ýä?Ù^{DCýMIXED4FGL J1832.4-0847¿âˆqýã	?ÇÔeG'u'À8¡å$w¯À:áî¶+ ˜@ºÑ!Vî@U™Yعj?ÁѨi@5z?å×p>×V>@áµâ¥|&?ÿž5e§?ßî*Àr÷C?ãµ¾=gêu¿Þ5B,Oê¿á¾QtfÚ*¿íáv<?A¿ïÿè«î0PSRPSRPSR J1832-0836?tŒ—'(B1?r\B"ÕÌ?æø¤Tf<S?ÆR8å'Xé?Ѽ"øo4c?Æ,ØyÙ?‹ˆ'±hÑ?"þ–ã¹H?߈Çz()?Èr°ZÀÕ?ߞl¡,ϱ?Çö·TÉ
®?±~ˆG~ó? ,…DýÿØ?àÎÕ½%(È?µTߦ$_?Ú²t(hK?µbH1?ŽHpõ$Ã?o$êÕ}I?å5°LIÁ?­	ƒ'æn¢?ÕQõ•?¬ƛƒŸI?p&Ašk‡?g½
K{?êß3j¡Åž?»¶ÁÀ̆?Ä)#ԊJ?»Y¸³ûÆ?|á&F?‡xgY{Ry?ß!,þï?Ì9µýÂ&ð?àE3#K'-?Ì"ß+°C?¥°"¾fÎ?–5gêÉJ?â<,VF?ºƒ¬»gþ?Ù…"úÚ?¹ ççfsU?im<¾×&§?Vì¾QƒY'?ç"ÛU{²?²´ÛÇÒ?ÐÅ
н?²Š-!€–.MIXED4FGL J1833.0-3840¿àÕÞ"#…/À*€d©ÍÄÀ:¬îÐ,ӞÀ<£éå‡ó@Z­KR8Ý@5Êd{?ȽÊ{cÏ?à%ô»ÿ/@î­ÕÀ­@{!]æ–?ïã.qÊH?åòØ?ɵ¿Ýè{Vb¿ä Ï§Æ¿î‰›ár¿ïÿԖũÃPSRpsrPSR J1833-3840?â]ÐpoB?ÃÍ_LtU?ÔÑQ–ˉ?ÂIJ¤$?¹Ì6(Iäê?§/–Fnr?æ|©Vى&?Æ@ÞªÎRç?ÊZ;)ÝÛ?ÁÏ'üý?·f°Ñ– ˜?´Ù>¸1?㌠øі?µd$ëzjˆ?Ѩ-}‰?³¼ãp‰G??¼"Wƒ}+-?£.YŽ?æ6꼐®?¦`58µÂß?ζ¿jõ¨t?¤9@ûÌ?±èÉÕz#?•{šÞ›´Ú?ڂûâ'ì?ÂÀ'([5R?Üb³ˆŒ?ÅHÎ<°×Æ?Â4¡+x®?±¼µ¬K'G?à
Ì7ëB?Íæ…ýÒÌ?×6i£Ý•G?Ìʎ4œÐí?Á[ûؗÊü?º¾(§
'Í?ØÕ^$è0š?·Å×z7Å?ÝôúÊT†?¸2ÞNª]?ÂkN!öõÀ?©¨Ð'UâÈ?×ÕBÈãšU?°	Ý3Ù=¢?ßZGcÌ?³× ½k¯?ÂÅßrÁ¾?©yÉP°6MIXED4FGL J1833.5-1033¿ìW'F¿ëù
ãˆÐôÀ79€C‡>MÀ:+-û»Í¡@—Э'Ñ@v¦ã.8"?§IÜÂ?˒Où<—`@ H,nóÓ¢?ñ¹Z¢
¢?ïúGߒ¢/¿ËYý¢W®=¿ä>ÚÑrMû¿ç
U=Ÿæ¿ë
+ãðU¿ç_QŸ/ÐPSRPSR3FGL J1833.5-1033PSR J1833-1034?Š:í@ÿ‡?¬ì9~Å»ˆ?Ùn-ì2©Ý?ÑIê[öB^?âÊÀ#è¤?Ñ3È:R"?"¹Œã"?Žiû´F?揞ºQg?Â[ÅvtÙú?Ò:ö$xÊ?ÂÐaVÝ?³i©½¯¿?¤AÈ*ßNE?ØcÊ¿ó?¸$-IÅ?áaIûso?¸v²!Xræ?\òN'?AO	±™V?ä7	H	Ì?«qÐÏQ<?×uç}¨!r?«'3áÙÏ??u԰᩽?†£IbøÝG?âÈâÅ1¢å?ÉkÍ̄±?Ú¿"ƒý??ÉNIJ]Ÿ?t=ú$´k]?{Òps-;?æ®/ê9«Y?ÇVáýÐ??ÒR¨C€ˆQ?Ç°X¢Y?¥ðͼn­H?›k+ö-7?Ü[ø_‰?¿yªw©ð?à›guÁ3x?¿­¸×ÄÅ?5‹õ¥‰À÷?$Í×uRe?æ+½"Hò?±'[½Õ‰?Ó£!ÛÐ~f?±Œ†ÖÉOëMIXED4FGL J1836.2+5925?ãŒÛ@­ð@9(€QÉ÷À53¡Qô¿ZÀ:}àÖo
@ºMϖ«©?þ$Ã9¦?X±ÊåWb[?Ù=¤¦=@_jcÇOµ@)."?½ÒfÛ)1¿ÀËFý¿Ûοì¹ñ¿åùèÄzô¿î¯Úê¿ïÿülòPSRPSR3FGL J1836.2+5925PSR J1836+5925?GãÓrÓ/S?Hl*³¾¿w?<¼ÊÝE?‰ÆIÿ<0"?~µ'
8äT?ˆÔ—1åtF?‰]*:ª;?°qJ–J[x?ÎØÿ?¸­Æw¶)y?Ÿ>1&C?²®Ë¯Z]?¡k¬ "ÚÆ?šŒÁÍrí'?ì®X–$'?¦bç5@Å?±×iãn?¡ ]ª–q:;¯¥½3)ÌZ;ïa\²s?ïÿý­%£º>•I>²•¤Þ¦>•I?WPó9Rnþ?Soߐ¹ç?ïªÒó=µÿ?ƒ.MåÍäú?'a$¼¸d? E
Zñe?€Ÿ iU?£ƒüÿc…³?îÄO³¥%?¼SpLe«£?Ÿ&"Ç?¹ýé6§?ŒÕ4ðå•M?Žc¦¬D?íÖ^Ú´Ž?ŸìÊ
í¸Ü?«dÑF÷8Æ?œÉ}¨pxÃ;ayÝ]qo;—'Óá}sÁ?ïÿzªÒ7V?AÃ1_©©©?ªžgôxT?AÃ1_©©©PSR4FGL J1837.8-0604?åBQœ/î?Í2¦ÆRàÀ7èȼœÓáÀ9¬DmŒË@ W\ÆT¡@öÙæÃ1?Áþ‡ÚÕN?Á8SX—›¾@t#¾K)Ê?ÿý`Îvðø¿åÒJO¯j¼¿Ö™5{aö¿à×:yx'â¿èRœðf/	¿è»°DÖɦ¿ë"^~»qÜPSRPSR3FGL J1837.9-0607PSR J1837-0604?…"¹SõÕÃ?†	L|Q׆?rbX£¦Öù?}æÞ5rÛ?ï"ìiRÝ{?"ÆCˆÐ?¤L…؆9L?­^—Õ"'·?±y¡@–™?¯B–'i"?ìŒnkx?¶S2/WO?­'œf¨€'?œz5?Ù?º\²2˜?§¿6a!>?êÙâŽCéÔ?«[:ßä?˜±´Ûxèó?w\<ÊÁD?žœË%£j¸?'ªìö‹?îEŒ X²?‹Ú¨<%žk?€Pÿ«€#·?ƒÅ'@8?›\Ä|sO?"]ˆWŽ—?ïxNŽa	ä?Ìâ;H—?'=\{Þ9?•ÞO$W, ?³˜
3"]?µTÈmzSo?ìûuí[Ò?·	ގàÁ?©ôþAªhv?•ü‡qñ+s?¾Dæ?q–?°‹!¾J?ê˜WÔ/ö?±Aª³r
?~Ð5š18?kºEàÁð?¡< 
Å'}?Ž]ùDôÕ?"Glž?|µClÙOTHER4FGL J1838.9-0537?Èï7t¥2?ÉzH†µˆÀ6é]…UÀ9¤ßI® @ lëT¢C·@÷é¾u5?­%Åask?Õæ͓œ*@'ڎO¹{·?î}Ððóȏ?ïh—c^t*¿Ý¤¯!k4¬¿árÞyzпãORúȉ¿ëÖWûi˜J¿íCèWlÎ_PSRPSR3FGL J1838.9-0537PSR J1838-0537?‡ƒÚF†Aæ?±âV—~pÐ?æéb£Iå?ʹçÉ8©Ñ?Ñqçù4E?ÉøÃФÉ?ndµ¸9g?|õ^×rãb?çª9ú͑?Â-×6÷Ó?ÐÃâ!6 ??Â@;!œ»k?£¼7 ¥'q?Ÿ7PGà?æµT_ª«?µ¹SÎR@¼?ÐÐ\Æ¡Ý?´"R::ª?ø¶Q¶Ð~?߁W&I?æœÕ~ª³{?«<V+1'Z?ÒÅEvy%}?«;Ø'±»H?¢ì"],œd?Æñ-"¸´<?å¸Ä?""?Î"Λë7?Ò0äõôŸ‹?ÊoÇß¹IÉ?nÉP¢ÏC?ƒÁ÷ yÌd?çèÿÐÛ$S?ǚ¦ö-ç?ÏàÛy°<–?ÇpïÁÄ[?•pç9X½ç?"ïlTöŸ?è	JI­Ñ"?·X:&v•?Í,¹òT›¹?¶Êrã‹ûØ>áØ0}°Ø‡>Ø×dãM?èós'
?¯ÈsÞÛ(?Ì1ì¿od?¯ÇÖßCs§PSR4FGL J1843.7-1114¿ïót6¼2SÀW=
§ˆÀ8Œ»*ƒÀ:ꨆœfÓ@³¸ʏ@FKùӖ?²Àßٙå?Ô]+ß×Ár@¼ó…@=rŸ.ÙÝ?ïÿºà¼ô¿ÛUçÞK$l¿ç™aOü¿è®¯?ôÖ¿ïÿûÎBÓ?ïü>>ÿðPSRPSR3FGL J1843.6-1114PSR J1843-1113?®Ûž5…~ø?´ù!ZìÖE?ä'Ö1Y?ÍԀqÈÜ?ÓŠ¦àï?Ì6NhUU?ț;3¡†è?Åv¬Ba
?Ô1ÀÞ=HÇ?Åfþ´õ?߀¡‡ñóÅ?Å$‰ß4À?ќ¹A³1N?²È¢àÆýö?ÜXÀžQu?´Â«U–¥í?Ò7ý®}=?®Ñ<I«"?É7óΪÑ?¤íË·-f0?е‰i ­Š?¨µ_¾nŸ¢?áW>ƒ{þ‡?­P'¬ö¡:?©?>²¬àÕ?©êNR@®?ä*2"¸ð]?ÊìòÃ<¼?ԃ³¦vª?ȹ¤œ,?­Å<K'¢?¶B$n/™²?ؕl@ùx?Î/O"ÎêÅ?áØøK£?Í?ˆ©åʨ?Ŧä6\Á?­ü¨ëBÄü?àÅ•BÇÑ?¸ZëhVF,?Ó¢`ºLcþ?³"ug[
?¨'yW	?ŽÚ"%âŽ?Öjx%ÍçK?µü.,Ù¿ß?ãJ'uL¢	?µã,¿v"MIXED4FGL J1844.4-0345¿ëÆTx'Y
¿ÅDÜþÉBÀ7ˍ¶6ˆRÀ:|TŠ›ÏÕ@ùà×Ù@ÌÕeø']?µ¬]–‰î?äï »ç¢@&W?·¥ô@8g'›%¿ïîB_Ëí?ï[Á&¦\ö¿ØÝ>|¿æàzÉʹͿî»ûXÑRn¿ïÿl\I¬òPSRPSR3FGL J1844.3-0344PSR J1844-0346?s£¤'n±G?wZuþ#)?ï™ÙóÒ?‡¥µ?p?ozEòÈ?l¥Uö"?~<ÿÌ;Êâ?‡8YVÁ)l?辐a6¦°?»f^6t¹Ä?ÌÖ}
þÈ?»AÒt=•?£ãH£'³?™ÁeÝÌƺ?遤"Ñ'á?±¢_ýˆÚÄ?Å›ëGP?¯x»C՛?g
FÌ3r
?P+µø"Á?é4	t?¨_×?˃¿%´?§Üÿ\Ýt¼?s…r8OÙ?ym–`õþ:?ïs‹¶éô?ûµpú9?‰ZY2ŽW"?ˆ4ºÉtež?qÂz>âu?{\ãî?ûÑ?ê<(´?¾ÃÂ7¡Ì?ÆziR©ñ?¾utKVj›?–Ùz9"ç§?"í'?êî—Oô?°þœ7?Ájs{Í«Å?­í½Î¦B?;ÖBóŒû¯?)Kµ{óyˆ?êøÈŚî?¨vRÏ}"¸?Äñƒ‡=?¨pÿ¦óPSR4FGL J1846.3+0919¿ï¢¯º9Ĕ@jš^»w:À8‹ÛYÀ;¦1Wà@˜–t¸@xs€?£×r࣢?à¸põ5¢@2Ôm?ž{@¤ŠM÷.Ë?Ëìւƒ(¿ÉîNý"õ¿Õà3œd¥¿â¹q:Õ¾ä¿îD žq¿ïÿlÞfþPSRPSR3FGL J1846.3+0919PSR J1846+0919?Vï-ß\'?T–?nî1?ï¸ÇB…qÖ?{¨cCú…?}à"R~??xÿi1
ëX?*3–¬ø?™ÚsÖç(?ì"h—ô?¹wO×Sš?¼ÇtÖ
4¾?¹a	‡_§¨?£SX&?œºéÁ?쒰€T½á?¦<4M?±áRyOf?¡ÄÜ"8?BÕñû"¯?7Ä|ò–?ï#9Q@¡?†Ë=y´× ?éG!"µ?†¸F:Éjó?`=JkU?]€'(p?ï‡6Co&»?¿þX%ƒ?Š#(ßB?‹Ù³².?!ê
_ñü?™ A¢Žj#?ëá:ZCîA?´ÚZÝyÌ?¿\KR?ÂwÓÌu?YÚWs;?˜•£äÍÔÈ?í2¡éQñB?£"àȞé?®(ô@PB?*Óv×?1;µÂÇ?€7§Õý?ï"¬{?‰vdWºÉa?w_J!é?‰oKÔPSR4FGL J1852.2-1309¿èÀi´qÀ"ý>" 
À:#º
RiYÀ<'@ÿ¥@žD 
é?ÿb‰,d?Æõì€Ç:½?à=òÿf}@{ùiãÉ@\u'ŸVG?ïö.Åæ(¾¿»òªÝ¿ÔH$ÜÙ4¿âg$ÒG`¿ïw^3'þ¿ïþº…¢kÐPSRpsrPSR J1852-13?Ìl‡"Ö³£?º·'#¿³ñ?Ü{ϑº´?ÄÚ®=Pԕ?ÕMì¤zë{?À¹qÄF%?ÎTFÜ»àÊ?Â6öŒ9?ʃ£­ï'?¼{§+J?áÊ,ànüH?Ã:IÁ®ÐQ?Ö0™ù™g"?³†ñÌ5£%?Ú¹ò5xC?´kFلö\?Î*ç¡Ü«‰?­ÆÐÚ.§a?àŽ
&"#;?¢*=Wƒ²m?Ì>ûÀw¡D? ·$P¯f?ÐÄgÒ»èé?œÿ'ßÕ¬ß?¶µYÀ³s?§8:1è?ß²×P¼ä€?ÅH¡¤ªï­?ڟÒ?ŸÊƒ?ýÉç6§Ô?½Ž²d/™:?º°îN@™'?ÍGqn,Xy?Ä«ü" ?äüMWîö»?ÇV¶Õ•?ÃÒOŽr?«Z à_Ñ¢?âÕ©I¡?¸¨æZá?ÐlšäX•Ô?²¶µ.+©ª?Ðý7C
Eä?¢ÿÄ-p?ÔaMJ¿—?®ž%ì	X?Ú¡{r3›…?ª™5Ô%MIXED4FGL J1853.3-0005¿¶¨FŽ¥aÞ¿Þz5›mYJÀ9 òxXrÀ;"!\q@ "Dû݆ƒ@–ÖZ²Ô?ÐoÜ†©'?çFz7Ԃ¤@Íÿàè@g ÎN¿ïÿõEq#?ïÿÙÔóü¿¼¸j•6|¿ÚÌaÿÏ¿ë3g5™?¿ïûÓ {‹PSRPSR3FGL J1853.2+0006PSR J1853-0004?º7€4mÅÖ?¶²‡Gíã?¼³Oý]'<?¹ Fzñ_j?é"¥úP½?Á«m¨5Ný?©‰áѲP?¬U[1l3?͛+r¨Æ?ÂVõôÓ?ç—'ä*?Á'0ÎmЂ?Ô"‡nÉ·D?°òPǜ ?ÄëÕ!kEÚ?©sŽ'yÝ?à³Ç@Rè?±ˆR3­(?ËC"w|?¥)÷^쀏?Ûþ½=¨?²½×úBö?Ö_{)·V?±ÀWsh›?¤|yí³?¡n¹ô'jz?Ô¢Ü/ã•?½\îr#Î?éÑ߁bô ?¿X´À=Ç?–ü<Ýôú?šuÌH²:?ÑÜY¿Þ?Ébaê*֘?æYñ7‡£?ÉF¿}Àz?ÇéÞ!ÞÍ?ª÷ãÖ"?ÊùäâÖy?°|T_3ßY?ãGƒþÒ®?²Y~5ZÃ?°Xb£«o?—¨%}±êE?⹝ðì?ºWõ
Íaâ?×£âsä9Œ?¹ixÑ=MIXED4FGL J1855.9-1435?¥¯Â¾À•hÀS# îøqÀ9ò".E©À;Ѿâ(~¤@€ô2}@3•#SÀ?¿.æâšœ?ÆӘ•±ƒ@®p:û~'?ýQ§Ù"q?ïöÅúJ´Y?薘ȹAÖ¿âê¹çíºƒ¿ÕÜH)¿ìD~‡Å\¿ïÿ*¸:n'PSRPSRPSR J1855-1436?â‹ÕI¯1Ã?¾ïäU£?³e(ð­â?©!C"ü?Öl€íâ?½ðsÚú?ÞR1V [ç?Ç,¥ZBÏ?±»õv<?«¼ÑÑ°?Ý>Ñj	‰?Ŭ5Ûё?çÚ§o´Ý‡?«ñ֍®?¯7Yî¿Ø÷?ž/'oHœ®?ÈNjÇk[e?©Œ9â3m>?ãs8wHi"?¥>¦ÎžN®?Ä͝³•ÕP? 2Hݬ}~?Íe€oH"¡?ŸÞg{z¤Ö?Û##)¿…Ö?¿ÃªÑÈ?Äd³q9±°?·. ³[?Úªƒ£¡R?¿Q@Øjî>?Ò´Oa€è7?Ç2N[ؙ?¹\Q=ùúq?·)'Jì?ãzN'€L—?Èf9°Oéw?âéõ4q?±aMJ¿—?¸µÐ.q¦?£;}0P'?Óþ¡‹€|<?°WÇßt'š?֞ù\o9?­m•¡ÐE?Ò-§¹Ôæ?³¡xðˆ'?×3^鼿?°9߉rwMIXED4FGL J1857.2+0941¿ÆðE=ÝíB@ñ|ƒ^À9B%ÁZ¨ÃÀ:àãܳʝ@=ø9âû@þ¥2?Ë°›=އà?Òõv¤¢X@÷Eî Ú@½"ñÙÍ?￶Ï4†¿ÜœiÌ2ô¿é3Î~}´a¿êæÿQ"W¿ì4q ԋ޿ïúFsBîPSRpsrPSR J1857+0943?Ù`ÑbCþ?Å"#]Ó?³ð½½.Vý?¾7³Jš®?àÑ—úÅ?Ƶ‹tŠ7ô?×MÐõÈ»è?ÂZþ5G?Â9ý{î?³ºÔŸ?ߢ'(X† ?ÁŠæ'4C?Ø,¯Zî?±¿'1mv?¼0¹¹Ó(?¥-é.m«É?àc'¾÷?²–»¦W3?Éÿ­ÝüӃ?šŒ_	Õàª?Èé'RG?œ$ú‰"*ÿ?ã~>¼ö?¡†Ý.À?Ô¤Q& ?ÁòoÔNKh?À-ê <,ù?ÁAî.‹?ᢁÏoá²?ÅO˜ È¢?ÀÎiã|_?·Ñpøp?ÊÇ=ÌiO¥?ÁtfØbh?å–¥¿?ÃNÍïþf?ËÇiÝ$™ù?«lÜœ?À:Gwkyÿ?©ó@@þ?äÿ"ªRŠ£?³ÂØà´éµ?¬`É5Áíq?‰%q|å›à?ώ+'Ô(a?¨á%ôV4²?æVhˆeÐÐ?¨3‡0ªOœOTHER4FGL J1857.6+0143¿éü%kc?¿âÓ_XU+«À9ÐQ¼‹6À; B\›âI@ ìÓRwò@'ß­*p?Í@zï_t?ïÿ¤€RuÄ@r²žM]?ÿäP\8åû¿ãú=‰Mq?ë÷u¢™r'¿ÙÓ7º¿åq"ý€Hæ¿ð?ïÌ+òÍ–PSRPSRPSR J1857+0143	?›Û¨îÝT?©<g‰X??ëÕ•¢œ«?Ã׎Q'íÿ?º`¡Y‡?Áùàci?™zþ@;?¥øRR?à;Ҁ.ÓA?Ê%ù=1þo?Ýöš²ß™?ÈãÌ¥ü'?Á"&õڄ"?¨HaÔiÚ?ÜxíAŒgW?³¿Am	x?Ú¼ÿC†V`?²‰DÐ;,¬?†bP f?p֎Êb)?é8ݜ?²PÏ4÷ÿ?ɹŸ€ZШ?²	"6)óô?Œf\!áH§?¯›?‰sTã?ì4†Æ-K?Ãd홺Àu?ºÎ¸E'l?ÁFߢèLÛ?…®dà]?"E´­*?ááOãíûœ?ÏTƒð‡^?ۏíª''?ÎêŸÎðq?µvôšÝkŸ?¤"ödÈAþ?޸룈?¶°É§årò?ÛéW6ó‡!?¶
ßän?U	
› 8Ï?GÜw‡¤@?ëZø"HC?²ÉX§u ?ÂmÎÞ°?±û¼*GPSR4FGL J1858.3-2216?àÙ҇nSÀ&ÉE•5†ËÀ96$)ªô5À<.wîN&Õ@÷ýÙµœ@ɪ`':P?²»dš‰X¯?ä:¾ÖêÞ@)¦XĽ4?ú¶ÛʚC?ïî"ã)/¤?Åvpõ‹‡Þ¿ÐYÏêŽ~³¿æØßT¹Á¿î @gNC¿ïþY¢2ÅOPSRPSR3FGL J1858.2-2215PSR J1858-2216?žˆÑ&L?ŠwÞµŒÒ&?ì"EõW°k?ߣ­Þcè?¹©ÿ9Óا?Âò¸yƒ¤?öƒœ°Žù?˜Æ\ý#Z7?ìj·+ÙUO?µv"'xn:?¸l¥¹›>K?´É¹ÅN¢Q?ŽP{
T‹Ï?ˆuã	gA?ì—b»>¸€?¨oé›\	?·zÚÆxƒ?¦ž÷´Ns"?cñ8) ¼Œ?P .Úùà?ï&"{Lsî?ƒ«üçRG?˜½‰"½ž?ƒ—>bHÄõ?€Hyzã÷?…Âúý;ô[?íÓO-˜G=?¸ŒkÈJèú?®¹ʚŠ´?¶Ü1CÄÐÕ?‡û¦^`ùä?ØKª$5§?íAÑñú®²?´çZ;å?²ñû£'"2?´U«Â¶Õ\?ƒÆf{g	?}J"È×NK?íC¯ú{~?¤¿Kž¸?³i³]Fv?£æ	ò~?<Í¥ôŸ\?,?ǚK®Ê?ïHF¹³üƒ?"BSeÆkÿ?–ƒò3%Ö°?"<C¼+ñPSR4FGL J1901.4-0126?È]qkÊvÀ¥úÐìÀ8©@GDbÀ;Ðzw@ c°(§>@™,d?°6{<6g?Ôz …2`@µGZ1¤¾@ƒG#€Ö?ìÀÂ}h‹…¿Ìo`¥aÏ¿àÛ¸•Ò¿å#'†Wv¿ëò"a¤	à¿ïÿÿ&¦³PSRPSR3FGL J1901.5-0126PSR J1901-0125?"ö˜¾¡h?'F6æ´?è¢ÞތÄ?À±%7®(?Êðå²ï"…?¾Ë鼶n?®Í¡ð"ï?­î·©á ¨?á!Õåû?ì6C!Ø?ÙâŸö·7?Á²À‰>úß?²¬ _N?£'J Ö~?è ²ïoÓ¼?²«Êëîr†?Ä'$5ƒ3j?«äà)uð?ÀZo]í\?"܇'¡?نj{&š|?Ÿ
S֓
Ä?ÞL]ÕâäÖ?¡TùŸ%»?ˆu…ý«H
?>¦¢wSì?êYyΣ¼?¹&éæZ‰Ü?ÅÀeÐP?¸öQ§Œ?šre…ÌÐ? ²M—"öï?âT@ąD?Ȝ°…ƒ/?Ù°_šU'j?Çîÿ-‹î?™Æyú×qø?"éšÍqŽ?ëÄVöJ¹?±P˜3^?À¸cÞ?­JYðZr?¤µ'm?K|†]"š?Þ_Ü·¯ú?¬Fq2Û)?ß"Q'~¹?¬˜D'HڔMIXED4FGL J1902.0-5105?ïâÿýYe*À6`Yž×ÇÀ8'hŒ±SËÀ;¯ð†nD@óœR†Šž@1¸YxAZ?¤—XP µ?ÑòñCú€º@(·×<'W†?ÿQK¯€á'?ìô'ßíæοÔíï\C͵¿ãÕ¥ÿ-¿æÌ£FÁ…q¿îß5/7¿ïýG¾Ûr'PSRPSR3FGL J1902.0-5107PSR J1902-5105?Ê]ýNY[?™èòôÞ÷?ì'õÙ¿;?¶šXªgÒ_?³ý¹²FlT?³­Æ
0'?¤¹ª="AÁ?¨rÏ­Ã?ì••EïE?²Iêm'AÆ?°ú¦8K÷?«d£Ðvœâ?²àëY–#Œ?£üӎ}žÌ?éåýQhÂ%?°.¹"Ô?½ï*%sÇ?¨9µíˆ?ŠbÎØë"?to«³kæ?í"h­
6?–m"wŒ?³ w}Ô°á?"²1ª—ϲ?"µþ
N»ä?NYÙ?ìû=s±†(?¯ŠK£
"?³8"àNF?ª
@=.u?™SÁâÒ·a?¦ýƔÏZ?ífZÀx?²íí#.ƒK?¬ðv8*8Å?®§¨û:?¨83<Z?žô¡¶VÉ?êöÒV›åq?®@Fòd?¼	Ñ1'ÑN?§¦"µB'Ô?hÀçÁÏÊ?V=˜Ðešy?í"s$¡?˜kyÒ}0š?³Ÿü±­<?˜êÊbPSR4FGL J1903.4-7053¿æÚ?¯îÀ:~¦Á HàÀ9øy5v'À<ºø6#@ŠøEÌgø?þ{9wÑ?·>,á_€ï?ã'Èâ\@!$¢v·í?ÿnãMß¿ëj2±‹(¿Å¸À¦MÝ¿ÁîŒe(£¸¿àfN²Š¿í™ÀÀú܀¿ïøÆ+$qPSRPSR3FGL J1903.6-7052PSR J1903-7051?™²O:SL©?¡…¶>è?ïlƒOÄþ?¢öÅ\ª ´?qQó–|?r¾û`°…?¬'ǽ>E}?­/ì;?ë½±º³ÖÃ?µ¶ºàÃÚ?³ÉŽKÂ'+?­'ÅÂ{ìß?µ*ðóImš?¥Ë>ÚÀ²6?ë–qBÚ½s?¨Ï(§×Ž?¬C	ï0éœ?¹ËÑÔ$?ÃƼ-~y"?¤jßq¼œ?蚉-»¥?ª½oÝišQ?·Å³YÝa³?žæPlÚè? ï!ÒXj?§…ívWΈ?îÀmÄ\C€?ªÙ*ÈéXî?xP,à(4U?'MW;B? Dõ7·Ï?¡©"dä3?ìwó!}Ü­?µàäݚ¢?´ìg™W°?²RË»ì?§וíVt?ÝT"®?í»>Œú?¢µB1Fק?§§t€]òõ?•â¨ëÁæ‡?¤ÓRÞ*_}?·.ЮöÑ?댴*-iß?§—k­RR?¹0µ=Y¿É?¤Ú8ÙÛì	PSR4FGL J1904.4-1129?à]´‡l׀À $Ï®ÿ\lÀ:ÇnìFå˜À<dÍßòC@}ÂuÛÏI@£°#HÚd?֋Óyq?ãRE|áÒî@~zÄÂ<P@¾ÒEå?åŠ)ýýÇ¿ì&á`'¡°¿Ôöǝ
"¿è€ôËۿïÿþó…õ?ïöÔþIœPSRpsrPSR J1904-11?å
=Pöñ?ļµT­xÁ?¤ÝgÀ?›ƒq‹žßH?Óh‰½i¾œ?ÄQ²|`ðþ?å>&÷ï?ÅkTğÏ
?'|Öß-2?"Nèlü²¸?Ô[䢁tµ?ÄpMî¨ó1?çáS–nÜ?¬W+òuV?¬ç·Wò9¬?™áÀŸ£æþ?É@Ùñè)?©5€¹Ã?芭Ö<$?¥4íJ²ê?¡¯Ã^†jŠ?'uM€W¦u?ÉiWÎYP?£šåtéï?Ù嬤…¨B?ÄƙŽÔ;#?­M`ùó?¥§"xÛN"?á8SÙ;½?ųÝR+?ÖàÃ7*lC?Èé´ÉÀý?žcú_Þá?£ Q`
?ãœ~'^f?É	0f‹`'?âºÚUÓÀ?²¹ú!ð?²C
÷£ô?ž3ØÍö"Q?ÕùˆÓ´Ù¢?²9wþ"â?ÝlRYû/G?²0ƒ¢Ù«¥?«r1U‡©?"T[™P@?ß%g{—Ù"?²¯ŽTj[MIXED4FGL J1906.4+0723¿í²ê\™wÐ?¬)¹úµÀ7Gg"s—§À9ÝZ±&~@ÔŽþ
2@%¸ m]Ñ?°Â÷Æ´?ҘnáµD@%Ԗ$š@°6ú*O¿ïcÔ?ïø{§@KJ¿å4>vn¿æº¯ßV¿ì£¶ôs®¿ïÿ#+~3PSRPSRPSR J1906+0722?gª¾Oð§?j™"†?îå,ÅäXã?§ušìíãû? 2Š•ëpC?¦Þ%
Œ²?x¢¶Ï?†%`'?ç²ÿh¢Î?ÀÇQî_C²?Ñt›o÷?À¼õZE×â?¯ÛHrõ?¡ÓÊú²Â?áћ®Î?¸ñ¬@ã?Øa`¶+Ô"?·«M®‹N?Q%A,
ò??pvPMp?ä5.?²{-.Š¢ž?ׄ¼'§ºš?²wq¯þ\}?e:Ñ|ÿÃç?c-À:Ó£?íê½Ù>ö
?±"*²c?°:¨ìt'?°ÓÑÇrÑ?rôq'EÃ?R튟è&?èvæ'Å0?ļ–q¤¡?͓†QŠ®'?ľ›]áT?¦È^üUIµ?œ–ˆ*!
?àÉ»Ê4ÛÄ?º÷xêCøu?ۓ|ŒÌ	a?»j3`»¾?$i
˜ùú?#Q÷Ž?æìƒè=§½?´,«Á7¸ì?Ò$k
ƒåí?´+=Ä9]øPSR4FGL J1907.9+0602¿éO'X8¿ìÔpÄÜ>À5äÜÊpÑúÀ9¾ÕöA:]@€Î(™Ò@Y9W9£?€×@ÕCz?Ó
Žÿä:@?Ÿ‡ð#ê@A‰Km¼œ?ïìu¿I×e¿Ô€ä+Ž#D¿áú@m®YD¿åÒdáÖõ¿ìøb²|¿n¿íãP!U*PSRPSR3FGL J1907.9+0602PSR J1907+0602?&Ùz+?Ä?(€Ù+«í"?ïXK0³"°?"Q"ÃMæö?"Èç²M¼ï?"@¼Œ!†Ä?n郗DÄÇ?Ä "£…?íYq˜É?³Œ'E'›?´='Ý"Ì?³)u©¬4?~Ítû'?ƒšGÇÀ?ífÒÓ÷?¥+2bºE?²Þ?³@¬?¤·´€³k>ˆæK:åàö>1Oxv¹c?ï&Z·}ý~?Åí¼Yا?›4œ–ƒwŠ?Åá'-Å ?0Žu÷!Y?$>;o䑇?ï ܽkìô?"ƒ'Ÿåµ'?›¢.NÙ<?"vðýLª$?`T¦4…?qŽÊåÂ>5?î=4j"œ÷?³ÉÖhÐû?«"è!õI?³šû×Êç?pr±>!‰?p"EcÜ{?°R?¡p%rypå?­ðñ1? çj:Žú¸>Z•‰èð>hê:-¼ È?îç㩈$&?˜6uÖóv˜?¡Ä•å'¾?˜6u
'µ³PSR4FGL J1908.9+2103¿îåЛ®$@è^ùŠ›À:7ÉÞÛÃÀ<Ó;{×@ÓÇ­©@±¢|—*T?ÄïL>h?Ü¢)` §@ö=Ÿ@Afl›‰´¿Àôš	¿çù5
¤¿«lи¿¤›¿åLx~–ÞÔ¿êáfµN+¿ïÓ	'Où=PSRPSRPSR J1908+2105?ÎÂiSx?»¡¥8«ˆ?λL9áÅ?ºÞŸæ˜X…?à  X+?Á´6RøJ?ÚAÔ¼+·?ÂV"èHw?¼;²"b?°
Ç8¡!Ç?Þ¯g<¶Oï?Á"Üaî¡?à/Œücyˆ?´‡épîëá?Î(Úa,b+?°x²ˆ"Ç›?ЌxÖ¢ÛÚ?®€ 6VSI?ã\‰à‹h?¢6N6<ÿš?¹ÐW'6'?"BÞ´¼?ÒÒ¯¾¦? ¿9Ÿàà?¸Âq¬7"x?©…W<XÊ?ϵD\²$?¿œh3£¤?äú`³öø?Àl>ç
T‡?Èì/s`ú?¿<µñq¥g?ÄË]¬¦Ö?¾ú"ôy˜?ä'áüΌ?à qD¶Ø?Ô¤$f?²?¼Ë8RK?ÒìIiÖ]o?¶lç†?Øo¢w<w?³ßê¹3ø?ÒóVûJŸÈ?§RöÞJ?Åߨº§cå?¨rµKž0z?ájS°×#?­}­ƒE=MIXED4FGL J1913.3+0905?ì˜ÖI3‹Ú¿åñ|‰'öÀ8¯YAºµÀ;0Ž=E@d"iS֗@ñÓíR~?À÷ß`"U?á
&"¿?F@¿b€þ˜@³8•¶Š?îœ"_ü?¿çædžJ ¿Ý %ú»r‡¿äÑiêe¿ïÿôÂ_5›?ï÷ŞÛ!úPSRPSR3FGL J1913.0+0910PSR J1913+0904?€¬\¿qŽ?‡‡þ8@‰?ïI%oȇ:?¢ò_ÿ%+â?
G@V=l?žmr=Aüe?ªÞÑÙjH?²Rçèuäw?à¹&«v¢?Æ¿—šåk?Û1؇7Ž¯?ÅP«•=?³^4Q‹ûÜ?¡xú
IØ?æD‹ƒ½u}?±"ÒG—
¢?Í>·ÇhE?¯	Ëïwߚ?£ÒQýë×?ˆ¹ƒÐ̺?㲟GÌ?³0jˆŒ?Ö!¤'"Q?²~'1?w<ÊhõÞþ?›'€DÖ@5?ïrÌVÁhý?¡ñ˜œ `?‡®…!'N?"¡KÁSÚ¹?Ž©ÙÕ4T?—v0w°Õd?áÓrBè‡é?Ì­2iT
?ÛcÌ«óA?ÌVc³rw†?¢°t¤-v?–taÉ)ª?è
÷̶Ÿ?±ÛÓÀèÛ$?˧æt¥?°HL;Ù$=?wd9÷ƒÀÐ?e—x¹n…ù?æÚkj?¸Ô;^}?ÓfºA¸d¾?¸"¼÷'ûXPSR4FGL J1913.3+1019?éÏÑm+¸§¿½÷'qøÀ8º(8-m÷À:gþ¬Bê@!¡žJÙB@& }¹i?Â6F¸÷?²n·Ù»s?ù…õB6Ü5@*ívæfQ¿ß`nŸðË°?ïò´BgXª¿×
¼;Ú÷ˆ¿å ø0'æ¿à®2ã'ø¿ç.uÉ°¸šPSRPSR1FGL J1913.7+1007cPSR J1913+1011?°¾YjË?«‡說?‰¿Ä<	ºw?"΂̦öÊ?í5Áq¾£?¯Gj·SÊË?ÀÄ%D™H?À©Ô*Ë@í?Œ9]ÈÝã?")Œ¥Ç"´?ëŒéààÖ?ÀæôžÖwú?Òøfiғ?«á2}?«ìÒ_4®?džI³{Ž?é\tđ١?­'Ì '?Ï·åŒ-¨?§hÁèö¬£?›Ÿ
§
áÔ?{äZrfHº?ç5GÉö·?§¦‰%´îª?³çL}L«?²OՎéòŠ?€Íƒ4-™?…‰!S6ß?í?àc¾§?³æ †Po7?µ@Bi"	?´'ð$•·?ˆI	mù—?"–IIã?ìöÚÓSWI?µ+–¯Œþ‰?½!Þ®îâÄ?¥Çoó[k†?£²9Y°#?"ÅzÈr?ë  "¾7?¨ùíù4?»èŒN‹?ž™ò5æ6˜? kͶ/;'?‹':¢1?ë|1š½í?¡ÛÌ
'OTHER4FGL J1919.1+2354?ç¦ÚðQ`@å9û¤P­À:µflE£xÀ<Š˜¨ØѾ@ÏÓ)`G@ãŸý`éO?ҀóûØÑ?ïü³åu:?@_–ž<–‰@£º	P¶§¿î«rßñm¿ÝiÚ¤¦½ï?ÞUIž¶™¿ì²ZÆ3¢¿æ¶õ׈¿ïÿѧ' ÖPSRpsrPSR J1919+23?Ü
Ù<FØ,?ÄáH ¾ã?Ãä÷â‹a.?¹:Îæ#ÿ?ÙÿªÓ†Wü?ÄqÖ9»–!?Ê1h
ˆø•?ÂÈdVä
?ԛ3
YÀø?Æï6ÑoÁ?ÞLía¾?Ã-Oaš­I?á'ÿÀ%Z¿?²¯S¿­šü?ÐM—*²
â?° ¾Îà·á?ÉXÒ¬,:¾?«cO?ݤHí?L?´!èÐ'd?ز‹ãé?¶J–?0½C?ÃRX¯,?ª{¦µ#l?Ðú=¹F?ÀoÍD?ÅvW•h1˜?¾'59h?â%K>æ÷?ßö·Ï1#?·Ä'ÎuΡ?»Œë¾Ýÿ?ØÙd
ý›2?Ì#ŁÿÉú?àš»À`ó?É·=¬¼i±?Ùû±ó©?µ%I"ã@F?ÖU½ªM¤?¶É`ãÛâ2?Ï^uI`Ϭ?®­ê‡J?Åj':4Ú?²;RD###?ã(yC7ã?À4=K‡_R?Íóóâæ>¹?¸~Œî'šMIXED4FGL J1921.1+1930¿ïO¡L…-–@ÃA2Ð7À:YP¦á€¹À;Ù'æ÷ñ@ 
Ž?w4@Ã/M= ?ÑcꠝCó?â©þk«@~Ó½Ö.@̸
Íóé¿à™æõlÿ¿èž÷ýR%½¿ÛõÀ¥Í¿ÞVe9q'¿íM,Ù|Þ¿êÔÁÔiPSRPSR3FGL J1921.6+1934PSR J1921+1929?Õf~)%¾+?Àž¬œg`?˝4l î?ºmêöûÁÏ?ÜÊç¡Ü«‰?Á֗NÄ;â?Ò°Í+±"'?ÃìíKñò?Àb=ñÁè‡?¶Ë·§`Q…?â	î@dõ?ÃUñúº?à•Ú4X;?²Þ>~Õ¼?ÆÁز´Ó?©6®@Y\I?ÓuóP!ß?°÷á^»]u?Ö÷Áq5?¬1Ýto?Lj="M‹?¦ßßH+f+?݆#Û|h?±ðÃd'Ï?Â8Ž=†É?±ÆhÌ]–R?Ñð…$Êæ?Àá³.<'?ây™ôÞ8Û?Á­tÕ??¶ˆãGĂ?³`A-×0?Å{ò$¨Æ?À¬«ÅHg?çÐ}-¨/?Ægx¬†?Ô¤'Sµg^?±
Ž2³?ÑʜÞ?³ÍvMR?ÚU¯®†Ä?±ì¿¸:5?º{«"eJ? BP¨'?В½2?¶ABYZ©?äuP¬ZN?¸$Œ{sÊÅMIXED4FGL J1921.4+0136?ïÕjT 'pÀ·rÁ¾{ÑÀ98èÑQ­À;Ù¥J_ @"ãð)ô@÷¨»uŒt?µ™ËÍ]÷?Òù,Ü×ÜË@M;ÞÓ_Ž@×£—'?堟²¸N'¿Þµý½ÛmO¿ßîÝBæ¯w¿ã¡¸LH
¿ë`0âvd¿ïï\ÏõPSRPSR3FGL J1921.2+0136PSR J1921+0137?²0­Ë>}?¯ºº—P°?ë›9ñ'(?¾]dtž¸g?µêõ"`~C?±°73?º$Æë¦?¹'ÇNnß?à3{kõá2?Å#[7;ß?Ù¶YT?ÄVIM9?ËÖ+'¢Q?±bP| 5J?â©Ìd?´Dƒ2Õh?Ìy'¥з?­Vh´¢É?Ó 'ç.Þ÷?¤®ê~W™?ßÛ	àmW`?¥ÀÞ (?ÊÈn¡ÑÕ?£ÒôƒDúx?›Á@_h1?"kâx;?ìw7ÙO?°ÛTó÷?µåÞ:?«Ä5Ü?£µ×çØÍÔ?¦TJ…†J?â˱"OAv?ʁfûjM?×ñáÜJæ{?ɏ?OÄ?¹Zڇ+ ?¦$Ýoz?æ?Ðk¦?µLÆa³6?ÊV_®Ín™?²&gä8ûÔ?¹¿©£§å?"l:Â?åPxö-e¶?­.U¥%?Î0¼Qe´v?«¥»½+ÍPSR4FGL J1925.2+1729¿Ûâðåk?æ'ÛçlÀ9ah¼O§À;:²<þŽ@(QغÂ@Ût´?Ê]?5Êè?ä"ûmI@9!ßyx@ÕäÎvE¿ÛxH[c}ÿ¿âÄôÉ_¿á5^Pp¿èõPPx¿í‰"Ô7û¿ïÿþó…õPSRPSR3FGL J1925.4+1727PSR J1925+1720?Ä2Dò^'ï?µàXX§N?ݞ²§Kw¼?Ã6ëf7cç?ØH*߅>Ì?Á-ÍZ	P?–Âûå)•?œšc•'ý7?Ê°ô—?¼Ä|q?³?èáÚG?½x,¦@	õ?ÅÛ®ïl4?¨;·½ÑD?ÓJm%a'Q?²`öÏzˆ$?àäÁ
 ë?´ɘ8;H?¨L†Ë{ù?†É—f£?ßÿp¬)ö?²ë.だ?Üöþ'7lË?²ê"¤î×ý?¨¶¸ñö?–MçÇ?۞\Ó?ÄMx"ø?஽5ç(Õ?ÃÎT_0o½?‰Ë
ñ4?"6èۇ`î?ËåFm¢›?Á¿ùÑM÷?è »Ú[è?ÁÀÓ&O—d?´S¬ÖÉa?šLü'Ó÷'?Ò=Ó~ÜmÃ?¶ñÑHouþ?äV ¥ýU+?·3"Îÿ6?€}.V3L?i"Àë¬Yº?âJj~à?¹€‡qE^ü?Ú}ƒ×n?¹f:VÊMIXED4FGL J1932.2+2221?æ&zÇ,µý?ùYº`úÀ9ÄN`	UÀ;s'È@½S¸cß#@Hæ=·´?Ó=`]¸Ã?ۉQÐ9¿@M}|,¡I@š@Zãü>?îÑÇ]w)'?ïý¶ÿÛíÒ¿â—DŸí˿刘ö«;¿ïܤ`œøÊ¿ïù¿tµÎPSRPSRPSR J1932+2220?Ñmýh9éõ?Äw6>Ã?¦hè™(|î?¡[ÒÏöA?åârÂPƒ6?ÅÒQ=¸?ÇA†äqjb?Æ|l%7i?Àwžõµ?µ=¡Cƒ£¾?æÜ¢òw›?ÇK_‹&Õ?јð`i'?®XoBX>?¼5ø'¢?¢"±_pïP?ã¬ÈÊÖõ½?±( !ÿ¶?Ê ôñrã? æ¶Í™ìÊ?ʏ5txoJ?¦^={?âÕÊe¥‡u?ª"Ök{?Á*¿9nê!?²÷iÇƇ÷?±»Ti¹?§q—2fM ?é"øÇ@_°?¸ÀÈím½?´kÙBiŸ?¸–—ª?Ôã?Åp(ÿJ÷?Âúw‰yç?èz—î>?Æ"|y?ÁÂ(¢C\?¢ T2'_?¼¿íl¤?¢õ€¿òR?è]ÙO5?«m›#‡nŸ?´Z1Áògâ?–‡ÝíL\?ÌyŒ¤
?±æ¡ï…\Á?æVVƒ
!?±ÇրX>«OTHER4FGL J1932.3+1916¿ÔœE~lö?µb©ëJÀ7~ÔÈCÑÀ:Ž•yy@•ŠÀÏ6@¬Ÿ€cg®?¨'¼«ë¬?ÛUߛªd@-ïÓh'1@>—û^ۃ?ɍQâ É¿ÐB3µ¿âé¤ÿ~Oç¿èÛӀE4½¿îf«esø¿è*AA¾¼>PSRPSR3FGL J1932.2+1916PSR J1932+1916?Yv·bÉv?\"çúó£?ï ¼ÉL? Wš0Bh?šQï?ŸXtñHÌ?{Ç"¦	ŸÕ?…²ú^mƒ?ê2©"–t?´Ÿ ?T±?ÆW ÛPr?´ÄN7 ?àå4W"?‹`F1¹P?ë؂ò|ùj?¬¯4côl?½¯J¤Ð?ªEo_"?5ª­fª‰¬?%ÉÀk*?ìÉk"ÐÃ?š†"B?¹žøܨÀ‡?š'¬ƒ†PÊ?erÖ)ùhÙ?i	ªw§µ?î֑Z—†?¦…_ôŸ0?¡?¼ô®'?¥M¡<à?q¯
ù'?|e¬>Ñ8Ð?ê飛ŒI5?º'‰BD¯?ÃÐ|V[?ºYx½è¶?>aºÛ¸?wñ"ÈÍ£?íwÊâðXK?¢E³GÓnÌ?²MÇÄ[Vk?¡ƒß,§§?î·yôµ>ý½ücÖ³º?íjµxûÇë?˜m¤U©?´§–_ñ?˜2&\¤àPSR4FGL J1935.2+2029?ì6{Fi¾,?°¼ÿ¿KôÀ8fpȍ£À:~E܃#6@Ú	Òg@±áYKË°?½(Eëf?ØPø€"Ê«@"³Ïà@{έw?Ôy$ä»ÖÛ¿ØH€aå"Y¿å¬:†
˛¿ì!ùOÖοïÿþÐñ¿ëÈ:a$ÞPSRPSR1FGL J1934.9+2031cPSR J1935+2025?çŠ'™‰Ã?ËG®	¾×?ÎôVQx÷?ʙ¦ÇKûÎ?—û?O@ó?šÏM‰	y\?·ô=°ñÆ?¼ŸÐH

?֓n›­ß¼?ÆôE
ó€?á·Àû՛J?ÇÙú^ø«D?ÑÁöÚèC?°‰iÁQÓä?Û*×Á¿ÊÓ?µeüov?ÓÒfGeLé?²ÿ"ý?µ`³·œ?"kM#¾?ÖÀ³ÀG"z?®ÁªÜldô?á󏼕??­˜"`k]n?ä¸#÷šÅ'?ʨVfÐ)à?ÔnQY'?ʂy¢-fë?¡
}þôÂS?¢ýíXÂë¡? ˜†˜6Í?¨¾C4A¬ò?ÙìvKÙ?̔ÈA«N«?â	¬¼Œé?ÌQ7ub,Æ?Ñþ?-ï?³Cbï%?Ý" ÇhèT?º&CÚ©?ѽ`ùj½?´i½IQK°?èÎø¹?wµM<9eS?Ýžã/»?µäO¥x­¸?àíêŒû?µ¢wã·+MIXED4FGL J1939.6+2135?âo'EM£¿ÒÚ
ã]Ý×À8â5~gÀ:Õoê›ë@.|Ì.lO@§ B•¦Æ?¿æ"´4û_?Új{ßI| @°lÊ-¶@Žg£'aï?ï²;†¾Ë'?׈Šþv=¿ã"~aÚ»x¿ç«Œ‹¿îŸ[O7¿ïÿý¡UûŠPSRPSRPSR J1939+2134?Šug¹ŒN?‹üƒÚÑ®o?íÁŠ…Ä>x?°{Û½jN?­Iý·ì¹ÿ?®_?¦j)Ã?«©!=?²`gˆu;?ÝÓiã¸:ˆ?ÀÚ°:DõR?Þ·rW¶JT?ÀªÄÄëï?°ce ²? Éè7~ŸØ?åöQdg0?µƒFÁ¼j­?Ïõ-<ê¿?²s03°xÝ?ž"ƒÃ	"À?zk‹±|ùÌ?áÈN?uƒ1?§ú|8ƒÖÄ?چDvsò?§²-KSÄ?Šþ¸B¬@ô?kÁÛ\Pœ?íĔ"¼ê?«\–oGÕd?¬÷¼el.?¦ò.'µ¬"?‹˜k?'é(,cÍ?ßn¨!Ð<÷?ƦMâ`?ß¹VýQ?ÆrªTÛW2?ž¦"Â$°Â?'ãfîÖÊÃ?èî]ðdñ5?´~²F¨tÃ?Èq·¦'¥?²§qX{Ï×?y}öîöS?aË¥Š‡ª?äb\wéàH?­THÿY?ÖÕO4=×?­H'XdMIXED4FGL J1946.5-5402¿»@ˆñ«©gÀ='…¹èÄzÀ9q0ž-}À<§'ÍÍ}Í@-µ"2@5¦à©ùc?°x±'ž‡?âÄ ¾{ü%@(ÐkYnL?ö	¸éžÀ?ìÔ þþ"Z¿Ôÿž[JT¿Ô·ºÁÝZ¿é‰²€ñ,(¿ïÿ«çy÷=¿êO]ë­¹PSRPSR3FGL J1946.4-5403PSR J1946-5403
?"ƒîØ'ƒY?š''ÂÅô?î€?GŠûi?²ºŒ·?›t(/™×Ÿ?¯p*lhŒ?¡`Htuä,?¥½I1z?ìϾóßúì?³nVá€f?°Ñä'¡‹?®bÙF¶Pg?ª¥ n¶?žv"GOh×?ê¯9K{(•?¬¼¿¯â?½yc ê8÷?§í¾:áóè?bfù6tʚ?M{ð¡?ïŠ%"×Îç?{ے½eÀ?ˆÜøùWm›?|í̂T?"®lÛ»?žm¸óQ?îð9Š '?¦ÚÜ$Ƙ\?Œ"ÃÌÜ?–B&Ò@?–]ôŒ=í? ûûu˜Æ?ìïFŠ[–²?¸dëRy?²î‡.¶`u?´Ùe–ÅšM?œ4:
žÝ?"°5RÍ?ëÒ;}äÐ?ªc5sñ?ºanjWM?§·fˆEy?6V¤q1À?%mì+KŠ?ï¤ÀƦn?È°Î3"!?†#9+u?¼j9鵃PSR4FGL J1950.6+2416¿Ãþ`KLã¿ò[vH[¹À9Z`,ÃÀ:Ño™\@ˆªFJ@Á¹Þ³?Êuú	?Ðеd¦GÓ@
¸S 8"¬@øᬭÈ{¿êÓà뽩?ïÿ$m'M¿ç`Jù"–-¿çÛ?áíEh¿ïüäW-
¿èü{±QFDPSRpsrPSR J1950+2414?ÉEëM&µˆ?ÁùU–àVÂ?˜7K=Щ?'0uøýÕ?èìÊÔ­Ÿi?Âj]'3±Ä?ϧéü¼_?ÀÞf–ý?³²Ð£Ž=…?¬í;þÆì?埫lˆr?¿cçñkg­?Ñ}Çw^—v?°ÁB	å±ö?·˜u'8)?¢ºXHCû'?äN
"	¯#?²/ðªèª?Ð/®{Jp‰?¤C¡J«€?À»ß‰è̈?—£ÌxiP?ã¹0àjù?¨S›/1K?¹ÐþU/Ý?´Ùí¤?—?ÊTÔA?	iâÒ?ìáéA]?¶8P/kž?·•!e°|î?±+0U>h?´ŒM¹^j?±ø0i?ê{Ø)»ÿå?·àGkãù›?ÁMŠøAÑ?£Æ½QP?·"þýað?¡eŸþ?è¼!¢Î?«gɒۏ]?¹Š;rÓÏN?šÚrm±"?ÄLJ⸂¤?¥_´kc«?绥ؗ0^?«|n¾ä&½OTHER4FGL J1952.9+3252?î!?ŸlQ@"™Iè^À6¨V˾°À:¤NA¬rº@G¾"¤9@a59°€?'	ÉSØ?ÑÏrä¤@<¤Y!…Æ?ü°ô9MS›?ꨏ òSo¿Ð"žry¿áÇggî%ã¿å¢l ºŠ«¿íB XÐ{®¿ì†XVÙ+PSRPSR3FGL J1952.9+3253PSR J1952+3252?>tŒÆ4?>‡¬à‡ås?ï,jpê?š‰¤ñöÚ?šÀæ?™Ëå–ÿ'Á?r˜áŽ~÷?"Úѳ>™?ìÿ]Ľoô?¶ <Ñæ"Ó?¶ÛƒÁ¥ƒ0?¶]âë§kZ?"æj?"í·ëï?ìdU%\—?«'v™<ç?·á«òÒ2?§šóÝnî>´î¥Þ^»>·g>UçØL?ï´9;œ•?ro$£"ïb?'ñ	¥j½?rn°Bð˜î?N"ÚÆÑu?J»zÈ?îÓÄÔ'V? ‡$ƒåI¾?¢SäK͝? F»|¥
?g®VÕý¶?z©¶dÛíÁ?íɇ Tm?·]ÅT‡?°úݍV˜¨?·Ê(?€L_$v'?ò¦ƒÀqþ?푉€OyC?¡ÚYo‹gÍ?±j#ÐJÍÝ? S}'·^7>'|ýÔ¯'>¢7_lDž?ï
3œB?'*ùn¼"T?‹ýVL"´?'*ãöåp!PSR4FGL J1954.3+2836¿çî˜'Q?×â4½÷ÇÍÀ6òçø¢=­À:{(‹9"†@ODL
D§@‹Ÿ}ß(ð?œC¦·©?Ô¼íÇWæ@4ÉîEÃX°@àp©?ï÷uýÞÄ¿Ì¿¯î¿à²¿-¿åÛibš)¿ìhÄÓTÑ¿ínúSPSRPSR3FGL J1954.2+2836PSR J1954+2836?B
FyA­M?D.6τWm?îåÿI‡ï‰?ª-W`Ü?¡WâPRäæ?©Ïäʾe?'B·œ!Pã?§:èý7¬G?êµÿ¬Ú$_?´5Šæq´?ÄÕÑÇø?²N¥ou5?x¿Ý Ž'7?}µÃF=]x?í|×r~]å?£X…Ší$?²F'¬1Ä?¢°Øa–Î?ªf¦?r?
VùÔÑS?í—4†è?˜›Ýº²xK?³ó0¬`¿µ?˜—‡Ð×9?P¢—ïžR?L£¹†àŒ?îÀŒy?¬´,Tã*^?£7"?¬xià ?n:='!¥?x	z£¶†?ëzR'?º!f %­l?ÁOÔè?º
»§­ÐÖ?q<†?f{Ï7ïÞ/?íÿÌeÁb?S¶céYV?­ßÒ¿?œ‡à¨"•'>èý[65?>ègËRv?í2ê
uNâ? ø'ì°¢2?¶gçÁîí÷? ø$f¼£PSR4FGL J1957.6+5033¿ï""mÌ@&	»j¤¹ˆÀ8eŒ«tqÀ;ϽƟŒ"@ýÁ@¸ýé¥K?¨®'zšÇ?威‡ª@5¤A»Œ2©?ý]!ŽpÅ?î݂AŽ?É¿ÌÝÐÀ¢G¿ãµJÐê°¿íP,h=Öû¿îÚG¿ïÿMéDÓPSRPSR3FGL J1957.7+5034PSR J1957+5033?TcÌ£Ê."?\ÖڙËb?ï=TŠN€Ÿ?ªåëoOC?—1ó®h'?ªŸ4Uu'ø?‹Äb&qÚ?¯Á÷»ö¬=?î
,ª$y?¶¢ù琇?¨=¤¬@g?°`'£&?¤ü7Fç¾?ãÊÛÓG?ë—ÃéNbº?¬¿UR[n?¸ÃÅe´Ø?¥üO¯^Ã? ݘèµG>ýl]èýñ?ï¸
ƒÝUí?q('*'ñ?ê~+.¢ð?qu½	 ê?V°§™¶Ç?W÷u']K?ï"Ð	¦¿?®³Æ/»	?šEô1éÒ¯?®g7Ӟ%¯?{~ø$\µ?'ð'†°?í±tZ?¿&ÌÓòu?°Ã¥;ü??¾+ÚòCC? ƒý÷:¯?š‰2'P.?ì)¹æ|\ƒ?«'*ݔ¿A?¶p2JE—'?¥áH4ñ%&>×_NÃã2q>ÚN>h²Èd?ï®]ST0?wE8å•î¯?"e¿[¤ÞH?wC	JђPSR4FGL J1958.7+2846¿ïâ6öƒ¡Ø¿ÖÚ
'ºÀ6ùgÉÉãÀ:—"rñ$@üi°ó¨Y@µ€e-?šþËD'?ÙoQ|I|¡@8‡Œ!áÒ?ÿd7È]?ïüÏ^w"œ¿ÄY€ú¼I¿àÁOÁs¿ç]*J¿ì£o÷à¿îBãÈÂýPSRPSR3FGL J1958.6+2845PSR J1958+2846?;š-i'½?AWTX	!"?îݪŒþM?¶ÿœ{'¨?¯¬"mî9?¶ãŠÁ´?sjÍ_¹ý?ƒ	"/O×a?ëöêPŽ?²ŒAg4‰Î?¿ó
µL?²i6Tã?y-ÀÁM«?€)	ÒObP?ìõ—VsT6?¥X0þŸ®?¶Àt2ø?¤Žy]—">Ö
Ú»—n>Ô«|ÿi?ïå]ߦ'?ˆïD³ó"ß?œóšõz?ˆîŒc09?M~ß9?A?T)²ŽW¦?î''MÖ*L?±ò"¶ët?­ߣډP?±¶†4
i?m7Ƹ-$ô?y€až²[}?íћFJ›?³Ç>ð
&?¶G´ïgTÄ?³ˆ®ªÙÐ?u&%qJ?vp'©òù?íMÀÁëa&?¥u¢3:!á?´?——ý0o?¥8æÙïü>ªI47H÷>°´øäÚn?îõ‡ÔŽý?'ñ‰£w? ¦
€¨#N?'ñl+†ÈZPSR4FGL J1959.5+2048¿ì5	ƒó{ÀÄ{gkÀ8Ú·ÿ¶.%À;Àäù}@´šýqÛ:@›ì't¹æ?¯uÝöjÖ?Ü UàÝ%
@%u"BJ'k@•šw?ïÿíUÙPi¿ºÌZ¡Œ,I¿âTI˜ÐEþ¿çIÁ/à˜¿ï-ž§öT¿ðPSRPSR3FGL J1959.5+2047PSR J1959+2048?‡9×Vƒ'?"ùøBáò?ìn,«ôT?¶ÃÛ*(_ª?¹¨¯à,ü?µhÚ~Ï'?ŒîÝl!ÿ>?"Ÿ"öÀ½Õ?èGR0×í?¼9Ÿê¸è?ÍØßՓ?»°`Åè'
?¦Ë¨*C/?›EÁ%/׍?é(™æŠQí?°ñ±9œ¤~?Ū®Z×ù?¯&£õƒs?"–
h¶\?xcVÄa^4?ìkg¤»?™Ácï	?·¢¿@[àˆ?˜GV=¿Í7?…­ÉMý"	?ˆ!Zè£ì?ë¸%d#Ò(?¹mî3{ŒÑ?¿‰¶ÙŠ9?¸~!ÑE‰J?€Êc.0?Š‡d'ð•Ñ?épüÉâ7?Â^º!Æƛ?É/lT<]?Â¢G4"T?™ö¦Ï?'­ÇËqˆ?ê@_nO"ç?²—K=Ü}œ?ÃÜ#rÜýƒ?±5`ð©Íy?l¸|}½ç ?U,ßVôÐ?í<TOk*Ï?›"G ҒÇ?µ7™¡s¥?šù®ª›÷PSR4FGL J2006.2+3102?í^z£y¿á<Âþí±IÀ9?ô³›£_À;p.fDØ@ëÏtœ@¬¬Ñ"Âr?Á¡Èg7r?ÚÁl!'J@×Aü#Ò?Ý#Š'ÇpË¿ïþ2Œã(?ïòX½[jµ¿ßՁ;ÔÂe¿å+ùæ/t¿í"XŽÛP¿ðPSRPSRPSR J2006+3102?µŽw«ôj?ÃQ†k¥§?ê‹o ŽÓ?Dž²&XY]?¶"¿Óü?ºfÉ¢?™OäÃbp?¬0ç~~á?äéªS%A?Å{@R«sŒ?Õk.^"'?Ä8¸Ò³°`?¿·èÓØH›?¬"Ï­·9¼?ã˜P"¿?´•Í±·
A?Ðáe–î՜?°* ã³ð½?";üÖ5ô?g±!ý"	?ì#ø"W¾¶?¡0²èY¢?¼N"æ7? ¥ïy†9ý?£¹Bp+ÐØ?¶Ê@*a?ëÀšìÍ?±?Á;ªMúgm?¸‡`¤3?¹{j»þ-?
b°£;?šdI=§$?äÝî{ÚR-?Ë´1É.eL?ÕÇí}OÂ?ˑ"ŠO¾s?°ØP{§ò÷? ºäA-}Ú?å{"8l¶•?µ_ŸnŒf?ÐÓ§o΢˜?²kÕ´¼…Ž?bþˆSo—~?O2Àµ	š?ìætÞÏ-Ð?¤G0ØDb ?¸4dŖ;…?¤Z«	hPSR4FGL J2006.4+0147?êd'‡žÀ/ŒgœÇK"À:ŠsùÍÀ<¬é\OŒ/@Š"Yé«U?ÿ4?Žò?ědŸç¼g?Ú·u¢™r'@ª•…7âÅ?ï‹x~™?ïÊ\ô‰?·ºä—ï ¿ÍÂ\ÜNõÜ¿Ú¨ÓÞ¹ß4¿êÓÜ¡@B¿æg€)ÙîPSRPSR3FGL J2006.6+0150PSR J2006+0148?ãvò«Ðö?È=²Íi?Ò͕œVYË?Žîø!?¹±ù¶¡?±†p"ïœ?Õ§ή›¬?ËTñ–R3Ì?áŽÐJä2x?ʹù¥6ʆ?¼ívn#ý"?¸ø¹&âë?ß['äYím?´ðÕQSûB?֛Ž¯cc?µÒSL°?ļÖ_Ÿ?ªò¦3 n?ÔizLÍ8-?¥Že_µ…?áe'öüºë?¨2ý¢°U?Á–ÃŒ˜ex?ž<'äeô?ÞЯË4FY?ƊÈàú{?Ù-'Ž§<?Ç9Y«!+?À{LHû>?´XÌ·ãŽ?ÄN7Éx?ÄÓyŒÉc?æç°¸f…½?ÊLCôæ5B?À­æœp}?¼•,ˆ°Nx?×/
[¤ó?¸kØÁ!É?Þùc%5¼?»ZCÿor?Åsò'¶J¢?® ªZ0Ç?À4rð9? îQ;bÖ?æ~qR±0?±[ºnÞ?Ç~ÑțK?«'î˜K&MIXED4FGL J2017.4+0602¿²{éw=Ô@À0Ÿb0vÀÀ8dÝÐ*OÀ;˜Å~ð¡@Ùtæ[ê?úក‰'\?¤ŽÁ¬æ±?ÚDãÿï9@5­¥¹bŒ½@/j¦¼î?ïÔ°á´»^¿ÁAá_¿ÌëõF";¿Ý¶0©7 ¿ëŠ÷0ÇÉ¿ðPSRPSR3FGL J2017.3+0602PSR J2017+0603?sRtŸï³ÿ?w7¨'Æ×a?ï6ß؝;?ŸŸ^TŸ¬?"O'šÀ²?›D:¿|?!~¯?§ÞD™bB?íVÀÒ?²ûn®²?¬ï[ ˜D?¬IÙ";Û?«'uÄ5 4?Ÿò|²ùª
?ë›çŠh
?¨Z#:V
?µÍR/'?£¿E$Í??6­"Íh?0å'{?î™u|%aÜ?'Ù¤,·Ç?¦;N
ª?ó\#Y…ß?w¥¶ö³8o?'Ñr-VëÃ?ïX(bÊ¥€?¡ÑdôçÂ?Ž#ÅFuÏ?˜É2¨7°à?ìùy©?š¡¨NÌ@?îDMP¯Š?¬L¯ž"FO?¥µ>©˜Ž?©MJ|5U?œGñ¶Z'e?–z²];Û?쭛š-pÚ?¤ßó
È1½?³&µ½T?¡tאœ±+?L
ۣǨ?ŽÉ5Y+é?î~êý˄?›¸H¹à¿|?®\kFèM?›°ð˜ñãdPSR4FGL J2017.7-1612¿ã<]©ÜæSÀ:4ÕÇGQÎÀ9ÎTæâ!ÉÀ<W^Æ^ô'@ˆ*Û Ð@䲁Çë¼?¸	{>d¿?ÑS•ÿ0LN@»Ÿ'x@mK–¬T\?ïê9>åîݿݒK|U;¿Ø¶<?@ˆ¿â•V©Zý¿íÂû'²ö¿änÒ ÷0ùPSRPSR3FGL J2017.6-1616PSR J2017-1614?äRZ̐x?ÀwY#˜ò'?ÓQ´xB0ý?¾~ˆ‡‰³?°&W¸»­G?žLÏ*cð"?ނŠ™v‰?È®Ø'e?ÙRö²ydp?ÆÄæ_¬=?ÀTýjEæa?°Ëgùæ?àÌá"3 ?µŒiÃ-¶?Õêìµïþ?³~
a¡¾S?Àù×IS†?¦‹Wâj÷?äÁ+@Ëw7?¡Põ®ö֔?ÌŽ"<n?Ÿ™âZKҜ?ÀäÄi•´¡?–;.ò_B+?ÒÒY&ŒÝ?¿(mÔ¼&Ú?âï"©‰&?ÁsEŸ÷¡?½9i²eY?ªëãø?Ò`k"goj?Æ>ºQu?àê¨,%ð!?ɸ­Ë0?ǔˆ&™`¨?½G
•Y?Ó-²žUõ?¶gœX)¦?á(õƒ5A?¸TUtí?Å7΋ÇQ–?¨O×öÏê3?֐¯KmÍÊ?¨Õ¼)yf—?ÚE綳?®×e¨"?ÎÀeT÷?¦†
UJMIXED4FGL J2017.9+3625?äb1_7aÛ?Øç;x| À7`C{ÓÀ:l«,i—@Þ$ªÚ3¾@ªY:-ù8?¦ÐNƒèú¢?á߁ëR@1í_‹Î@¨¹(«?j•ExZ/¿ÚlªMF¿àPhb¿è¹¿èîú‰žyÓ¿ï4ör2M¿é"—VÉ:qPSRPSR3FGL J2017.9+3627PSR J2017+3625?tOï±*7?~zdg…Ž?î$®3&?¹Z³–#(?«4'=ËVo?¸(ž3 ,µ?y«°é["¡?…1vUØà¾?éÛêž2ÊF?¶ç·èË?ÇÂ÷ÿÞû?¶EÓ݂ê?™oöWì˜H?"×÷»Gp*?êZƒã¾šŸ?¯ü¤ÏÚR¯?Ãgñ¥c=?­s"W'•>?$ÄòáË6?$Ôc¬Þ˜?íQ¤ÆôF?šI#4{S?µlÈa¸i¯?šCX,Wp?hè@†°ñ>?qhŠŒ?îˆk±s?µu³ Ù]b?¬Øõ:"TF?´´B^S°G?q—¼VŒ?zø·¥µê?êÙS¬."?¹0e©‰?Ä
öâ¬?¹öåRQ?‰ÒÐ"ëÝ÷?ŠÒÿF½?뵍S÷4;?­q¡XÚ։?¿;XyFq?¬Cã)''>òÛMBY>ëÅ;B‹?íà)ðX1?š
®o@Ê?°ý'Æç?š
*;Âí´PSR4FGL J2021.1+3651?ï‹Õg'?»ì˜ïû{À5^Ê÷àÀ9¿-<y-@îý­•O@âXýÈ[?…\¼!6?Ձòžm"×@J^$_ZÙj?ý|$C?ÞÔûD"i\¿Ða1ޟ](¿áLà«üÉ¿æW~6fÄZ¿íZhµËÿ¿îqžBuÆPSRPSR3FGL J2021.1+3651PSR J2021+3651?]Xs¸¢1?—MðX*)?îà'@×-?¥Ø!\HÊ?¡ShDÓ?¡áï[³~?o'VÊ1ê?
ºÚa(ó?î|2?>ø?¯nÕµNŒó?¦C¶§7Ù?®$M;lô'?×¾œÒ(?†˜ó`È2W?í¶.¤œñ­?¢éºZŽ©Â?°"Þî×?¡‹ïfCš£=±§!X®˜=Íè˜ñÉ?ïùÜ·Ýî?M0ؚÕ?H!±6Ù¨?M0ؔÈûº?~wJW›¬?µ"N\b	=?î¶Zéõ@x?µž4T™«? Úrÿ"Ž?œM
Pƹ?Z4 Tôx?p¦&×B!?ï%åÊA#®?¬§ÿNYsG?™ ¯Ì'¾?«ù¿HO±
?yó<Wß?³GS€Ž?î%	ƒó{?ŸUà|ïú?ªh§Ü˜ëË?F'¢/Šõ="AùfÑd=³à
IŸ?ïí(9&‰¤?q-VÀ *?b×ǯ+®?q-V¿p>PSR4FGL J2021.5+4026¿îuø#V‹@§~¼ž`À4æe×Ë-À9E¼Çœd@̧"W`9@èEc·_}?‰ñЁ&?Ù~†TB@Lôów[0@nÇ­Ô¿Ñ&s1P¿¸{w€Ñ1ò¿áÉ^ƒCÿ¿èU±|æ¿îÔvå9«¿îõ_þmXÉPSRPSR3FGL J2021.5+4026PSR J2021+4026?²(@Ï0²Ù?¹øÞV?°?ë¦qCd.?Ç-£Àë¡?´ê‹§"8?À
>ñœ(Ú?tviے?º?FÈt"	?î+e‰q®C?ºÖÅôìQ?ªºÚ.zµÕ?¹";Ù?Ê?'²I¾»?²˜Lµ·È´?àÌi	{K?µÓvæår?ÑGÿÔÈ*?·ën…ç=Ò"M~êv=ö¢n±Ëë›?ïíR¡Á?wkïiê?b­^(ôzÅ?wkî÷«-ý?¬µŠL/ê?²,_úÿu?ëV«Íà?Ä e[Eî?¸ò‰åÓv8?À}ՉÅø.?rYò·Ýod?'Ò×jïéÜ?æ]?½ƒìý!†ì?¤ZSFn¼[?»p‰(7Š?Ǹkç?³ˆ&i´=?àœøèÎNò?·g
üã^í?ÒéØ®#á©?ºRû÷ =€]*ÒÀ=Ÿ«k©;Ž?ïØtؑs}?ˆâmìï6l?sœœyMÂ?ˆâmìï6lPSR4FGL J2022.3+3840?¼UP©æ˜Ñ?î=oâ'JÀ8tPrßÀ:‰ƒùdo@8'l+w@i_?*¸?¾—R£/š?Ú8ªkxõ@©×ý'w>@,Á®
¿Í?îZná_+	¿â}]"ðÅпèrçÉ0`¿ç¹" ]îs¿ïÿë<ú\R?ïü›¦2ÚPSRPSR3FGL J2022.2+3840PSR J2022+3842?«Œ2Ƕ4?«~´NÇPq?êöÈ\-[?Ã"Äj%?º¼÷S½?½?Cõ°?·'ý¿]?¼Âa×ééò?Õå>"[U"?ŘOS‹?â4#?ÆÉ4Z]†?ÈĤäj<#?®Y
Ÿf<i?Ûߨx|
?´ÌB#ÁH?×¾©æeF£?²"…X('î?©Ël HQ¬?ŒT(fʑ?ÖÚ-Y:À?­.Ì)æb³?âö2‰•¥?­b®'qƒ°?¢ÑE˜À ?¢F*k?gj?쯛ÛW?¸ØUV	"?±:¸'zߓ?³]Õ!ð$? p 5›ì?².»ù0|?Ø*-ûæÀ¿?ËCÙ,ÆKm?âêÁø22?ËlËôúW8?¿Ò™nÀ@ç?¨K²â¿$?à­Ò_&S?¹£VF]²c?Ö¯´æ£ ?·ö¢ÑT?€ŽâOЫ´?j;]àA/?݈ìg
À?¸V[ÿ ­·?á1çí¡?¸0>>¨RMIXED4FGL J2028.3+3331¿ÜÞÒŒâÀ¤‡3eˆÀ7™ìløÀ;7ý˜F³@ļ YÒ@'ågÎE?¢1R»í4)?䪘Å^C'@8c^t)ž@úúr!…Œ¿è0SðBÛ?ÓÆìM›"F¿ÔôÃ@±öÞ¿çâP¢Yܕ¿î9Pƒ¦N¿ïÿþÞ÷PSRPSR3FGL J2028.3+3332PSR J2028+3332?p¡"bÑK?­`0ÄÓ`
?ï·=VÖ.(?­_âcä`?s¿Á5²Ù?uÜ)õ9'ú?!¾¦ÏN;?Œvø5Úx?똲dk.?³Ü8òÝ$*?À¤(zá˜?³Úô>ìÿç?ˆ—¸Wš§©?Šfþ¼³úï?íï4\½n?žÉ7Óîå?ªæÌ5±6?šñܯK*>ÝÇúÏ>֕
°Cœ?ïºÀ{ŽIb?q"†5ì¹?L>W3¯Ž?q"¬0Ô?ÿ?9c¼¿£?6«_û1"?ïÑ6·TÉ?€€381
?uÎh€äkK?~{1±ITÛ?u©w÷ ?‰*8Xy"]?ì<çù	R?¸¦NãÜÁ‰?º.)}>?¸fköª?yTzõ¥?}—ûúÏÅ?4äto?–QË6»!*?¤=Lñ<R?"ÃϹke>«¤j¦ú>³+¡f(Õl?ï»W¶Rë?tÆÉ ðíh?><µïà?tƤ:ñ'RPSR4FGL J2030.0+3641?çò¸áªÌ¿¿÷ ²BÀ7ìºç£À;EWøåZ@ÖâVÌÀc@Mø±W%?­Fk\?ãÛ'8S-¤@1-û¹@ÂC*8ä¿ïsÎ>º?ïþñ­VåÀ¿Ò@묋å¿å)µ/ê©¿íñ™ O–@¿ïÿý`éNäPSRPSR3FGL J2030.0+3642PSR J2030+3641?=^W\³ä6?J¼XpÄ=?#ÛÁ ?˜õ=ô4ù?Š-"?Ðæ?˜Gµð> _?…&y_"? ð²óòPv?ë	˜µ»[?²ÛTçcº?‰Fçžú?±µvÇÚ
'?ˆ ¡ÃÜ#²?‰Ã…r½"'?íNÑÞ?£«åªûg?²‹k¤n?¢¡Âsîº?4<%}è?%Ê…\?îš>pN?ŠM¢p
÷=?¦3¦­?Š1Äܽ?IVn#ÿÇ?T´ˆëÖc?ïKžþ¢!?žA‰ŽéÐ.?‹¢Ó%?5u²ÓŠ(?|ޅȈšÆ?¥C4M‰?ìG+ÿsy?¶ñ&û?»ùÞA®?´ÿ"¿•Å?|ϵIuWW?€Ïì®®›?íó0À"€š? š¼bÕò?­2ýQ{§ÿ? ‡—©ùe?ñi˜)Áí?sÅr=®J?î¤å><À?Z'D»¼q?¥©7áqv?X;hQq9PSR4FGL J2030.9+4416?é1?Й@%z
XÀ7ßÉÇ^ÏÀ;(öýø¾Ã@Vv&LðÊ@Y ¡`7?ª'ýÀ'%?å-‡ÂÁ@0¨…<ƒE?û#H÷ë‰{¿Õ!ΜZ¿¿Õ{½ZéÛ{¿Ûúd_¦¿êŒY?¿ïùºá辿ïqÊG·N¶PSRPSR3FGL J2030.8+4416PSR J2030+4415?bÆð¥©!?uù¥]ö?êcRyŽP?ÖÝSâD(?ǖ™Ó??Öçkð+Õ?…Õbº¸·½?¦ÃoõP?êè9a|‰?ºV'#
?ÃÄPQ|?¹i´B‡?Š¬[Jûè?‰…õ–Ó=@?ír?à"o? ¼k®3`~?±-Ro·¾‹?ž‹½nþ?ÖýóÉ?åk~z²?ïW°kP)?
}É?"ô¢>?ÑàGQó?YúÎË<?d~Z=Ùw?í5çS¶¶?Ɋ
Kn¤Š?µï•ŽB£?ɅçډÑ?ohx]‹€º?|ß@–jßv?ëE·‹-Va?ÀŠ7~÷Ì?Âkñ¸û›?À…‰,Ó·?zÈ¡_,֎?yl[뇦¿?íí;¢\P?ÜŸÌ´Z?­ÖxÖÀµ?œøêg0s>äXo®7<¹>ÝXŸh4Å?ï|ïW™Íz?¿Jü#6Ç?_‰ù¬—?¾SÇ>PSR4FGL J2032.2+4127?¾Sòà «`?ðbá& %9À6ªŽÊ2¾™À:U»¹@ßuÚ!Ê?ÿ· ÈÍcÌ?žYÊC'?ØÄ6Ûß9a@7ÎáXu@7M­ÝÉI?èµólsÆ¡?££ä¡)ÛÇ¿ÕP<ÙO<¿àR©»OÌÇ¿ë†=Á×{R¿íIš³uòPSRPSR3FGL J2032.2+4126PSR J2032+4127?c¯P–ïß?hì|ýA×?íÇ)Si?³Üûbõ3A?±*|2.-?³lŸ4'Ø?wQ͘ÇÜ?ŒÜ·Ÿ•¼R?éàÔ®|™?¼a"âåì?ÇÂ!Boç?¼‡íµ$ºu?¡‹êä¢Çå?šBHFb1p?ê£@ÔM9?¬xÜôWî8?Áô¤?©ºeå3·B?²UÅð›Ð>ûNðɀª?íÇr&Qè?˜Š
ŒID°?±ÂX"ÅYã?˜ˆÒ;G?g"èñk˪?gÕô'eJ?ìýœ»• ?¶Ã¸"ƒ¬?·[[Ôé±?¶_;M–³L?n&íô‰»?xà=—6$A?ê͍ xA@?Ârœ¢¶?ÄQ-Å
5¹?ÂuðKpÛy?š¤*Ö¾P?–›ZíjÝ?ë§g½Jñ?«
ьÀ'W?¼·^¯Š?¨hHœY›>ف'=fý>ß<_2WH§?íW§Xö!?¢ÿì.ÈÞ?µB_8œ??¢Ç'ºPSR4FGL J2035.0+3632?×BðØEðÀ»K›	bÀ9 ¨,"	À;Ý©Çå@'L
QÍ?þ°ð˜ƒïä?¹§µ\˜²?ê€ÖõD»@(WšÏú@ˆA¿ïÀ‡—ů?ïÿ胸›?¶Øíþ†êQ¿ÙÒ¾éµ:à¿í™pŽR>¿ïî$ïßvPSRpsr3FGL J2035.0+3634PSR J2034+3632?r§ï¡¿?rËÆÎf?í'i­ h?¾ß=µ·u?¶¸íÀvøç?¾~´Ùï}¯?…¹[€Ú0?'æ§XO¦?ê/Á}}&?¶)usŽ[è?Åïþuf^"?¶8"'¸?§ÊÀ‡é<?›ô–Ö Õ?êUÀWY¿J?®÷žœ2²?À¶NŸäü?ª¨"Õ?sªeø™X?\.0_YYö?î 4?'/,¢Ò%È?«‰¹"Y?§Ä´mq?}Ad$?|"Ó0¼ÿÜ?í¼ƒT™ñi?·]¾L+}?°GÏ"ï?¶+àåzÇ?{¿Ù£º¤À?òN…ÙÒ$?ëF¬ÀÎøÝ?·óo»3­?ÂN0˜+ä?·âë¿æ'B?¡–›¾[º?–öâcÑ¥h?ë%ݧ»pY?«K–@?¾Äá­Ý?¨oËÛYYB?P´^nXÎÒ?B1K€iè?î‰=_Má?•ìéðŸ?¦æ‡ÞDÿ?•C½{s_PSR4FGL J2039.4-3616?ïóûuŠNVÀBEò×sÀ:`
ôGÀ<œ£äv6¾@­ùÄ|œ3@Ží¥,u?ÀX[
è'N?Ù©íœ@(R. ý@–ÖÇL…?À×½ìŠ,¿ãˆÄvW˿ڟ[O7¿èŸ5_ˆPÇ¿ïþ£ßm¹A¿ï§匷3PSRPSR3FGL J2038.8-3613PSR J2039-3616?펷úhøx?§å§"MJ?¤êMë_"ê?¡t+•Ô?¢*2p¥
?•Ãò¾æÃ?ë
lat†‡?º¡Ù}'?´œu¤Ä[i?³»
vp?²ø'PáJÜ?¨o!"ží??æVŒ}§K?±Øõ­Ÿ=¦?ÆÊ
c
ôé?¬M~uí;.?¿»ÕöÛÙ?¥
Êþw‡?ì¼ÈöJí?"l¬M;Í*?®½5VÙ=?‹,Öz™¦?¥.ú¢?‹öUl«¥?éó«ú!ø+?»Ï<¾¢<«?¾dn>¡ü??·s
>Á]?±þ1î–tl?¦¯…:Ó@?æf6UÛ?Å~ˆéjŠ?Á÷^ÏKà²?ÀèÕt™¹?ÄoÇÙHR?¶‹kZ0?âW‹t?¸ÌÕÍz½N?ÑÇÐ[#?µ|úN]Ó?Åg2Ýwë?©XçQ!I–?çbÅÖþâ?¬	Ò‡G.?Ä7Èl"?©p4f&4?¼z@oÔÁ?¢
¢ÌAcWAGN4FGL J2039.5-5617¿Ù9ªèî¸ÒÀB'ÁDŽPÀ8êÀ<Èe^ÿj@rŸÚ¦T?ÿ©D1ˆ8?©Ólà9Lc?ÎSíèÑ:E@#_'`4@6Öd¦à¿ØE2¤—ú]¿ÞÏ|_LØ¿Ýhã«5£¿âfB
f‹¿ííC/)¹7¿ïÿùëñPSRPSR3FGL J2039.6-5618PSR J2039-5617?àGð4¨K?Í0£Qåa)?ÜCÏ%u8?ÎÓBVUð?©pwÒȋ?¢cXb>Nõ?ÐbÇF?Ê' È{É?ã‹Ú-!e?Ì}WGQ?ÂéÉ	Iá?¹&oœÄ<?Ú_¹õ•Ôú?³Õë¤U?Ý»EÙ܈_?´µnœ¡Óþ?¿"Â6Šš?¦©Ørp«|?àl²ý‡™?²QÒW©žÅ?Ó~è•w˜_?®oû"}û?ÇObÜ̧Â?¡ø3‡Ñû?ÑO›(ì?ÂÙ1Œ6|
?䖐AÎxì?ņÎLöö?¶
P(o1?«#Eiì'Ë?À"ŒŸ59ô?ÁBìI®?æ—FH
à¾?ɑˢˆß?ÅZ@"C?¿sWOƒ\?Óó¯òmèˆ?·'Ȳ5ò«?âÓT%q)?¸^àø 1±?¿š¥•ԙ?¦ìÖ'u'?эºAžŸ­?±ë œtÂ?ÛÿG ®~â?µ@(y-ÙÑ?Òrþ²ár?­
"†ùçŠMIXED4FGL J2042.2+0245?қ¦ïÃqÚÀ7	üȽÀ9Ù©?ÿÊPÀ<QÙŽuy@ðªÏ÷Ð@x½ì_9K?¾­odfÜÙ?ä"_¾+Ÿ@@ »'-ºMn@¥P<³?ïÿÿ^ðP`¿×QN¼¦Žõ¿áš'ç°ë¿ìúE`²Ge¿ïþú¡Ç:'¿ê–­ÁnʹPSRPSR3FGL J2042.1+0247PSR J2042+0246?¬øGM<5ö?°ëMˆ4q–?íê¡kl'?¶…Óô²š?¡I˜eï?¨$0×{a?¬8ªë¥?®ß6G>÷Å?ëÖSÈ1»?µ3¸Ä¹I?³3c^
V?ª§¡ˆ(s?Áÿ΃þt1?ªîó÷µ¸ò?æqŽÏªçd?±ûl苚(?Ä9ö?{¯¾?©÷a_' ?«ìÄÊÍ?Œæ1€^<Õ?ìÞؾ?œCy‹ã÷¬?±Ò­)¡í"?™1H!Úá?¡ïRzŸÀ?«Yë/˜±Ù?í¿‡ÖèHm?±ûŒzb¡Õ?¢0§l?£|·ý?ŸÒh¢æ'?¤=î
"\&?ì¯Óa"?¶ÎÆÙl
?²ŒÉ˜ À?±»ÇÈb?¶º†v)¼?¤Sz aM?ç뾞¥‹Ú?³/Ýo/®?ÄóÂJùߑ?¯Õ
w² ?'Ͳ^yò?g°S-È9é?í¤@
ƒ˜ž? '^
CÈ#?°"IA»¬×?Ÿr6>°ˆ×PSR4FGL J2043.3+1711?ãvòôþ­À.¢(D€cÀ8H…'òQÀ;½·ý1ïf@f­ZÁ—?ýÿ´€¥¬Í?¢sz ,›??Ó<ëƒFF
@0©:÷LÓ@Ú>›ò{?ïÿؒӬ»¿Ó³ÚøßzN¿Ù Ú@'ãI¿âŸ>HÀc¿ëò¬MÑD¿ïÿÿ)@k*PSRPSR3FGL J2043.2+1711PSR J2043+1711?œñ·ùè?¤Õ"íÑæM?죉Û>2H?·z ]—°—?³§C)º'r?³wô*??¤¬÷: Ǩ?«ƒ'O±Ì?ì‡"ij‰?¶¤Z«±Äë?±pqUe?²-ü4}çá?œƒJ³é3?–Rp5(H!?ê~šä·
?­Y *2|¬?Âu.‹Òî?ªŒ¯Lõ?xÙçt¤?jÛÚÝ_ÚÅ?í|Ô3¦ÿ?•*H±}C«?²'ãÁÐ<?"(]¶!a:?™±®¦U›'?£±~Ž€?ìqÚ×b¹?¶Œ†{»ªi?¶½z'Ñ?²Ëe®*?–¡Ìoº
?œ\tí_5è?팁½§7^?²#åfMq5?«æýìӞ?°ãýí‹q?Žçà|ª?¼鑑~?ë·
î›?±ÿýŒïM?Áâ²$³q:?°8añ6¹?^"H@éX¹?SðùŒÿCv?í Àeœx?œa/e‹Y—?·¬Ú"§ž?›ö6Õ3‹ŽPSR4FGL J2043.7+2741?°A©ìÃ¥@À"Jeà.©aÀ9sZôB\œÀ<%ê°¢¦@õ'¦¸'@+e˜U?¶'«hÎös?áëaŠ@ ö²(ܘ@ÆÞ	àÿ¿§˜»"Ujk¿Ðg°Ql¿ái¬}Ãû¿ì¬#ßÙ¿ïÔ÷©i^¿ïÕ@¿ð©PSRPSR3FGL J2043.8+2741PSR J2043+2740?×ÄY™¬íg?Ë<·Z8Ÿs?àþ]meÖk?ÐEÅZ›?¸û®-¯£?µw¿c¥?¹ÁZµ¥‹7?¾š¼É
id?ãƒ)hŒ¹ë?Æ8'¡5wå?҉V})]?ÃDâŒkwŒ?Ó#¨ý æP?³P1£×"8?ãì¿Hª¾°?µò¸¥A?´aÅX>? êÃÊóîJ?Ù|ÞA-5²?­¾Œ‹FÎ#?àû§««?®(žÊNûã?¹\©»È? <¦·Tå?ͪòì_þÝ?ÃÍ<&y;?åöþ<d?Æl+wR?´ò(Dr??¬k½N<?¨{é¶5³?´MhÇg?åË=¯:@?Ê´^Œ'k)?ÑZ!@ŽÝË?Ç©{ª?Ñ}X÷¤"?³Y€>Þö?äù|¢?´q9¼8a?²BpB"An? ÜÙRtʋ?¼÷/Ù®Ôâ?#­UÏp?è&POvÑ?¯EcIký×?Àë&×&ºK?«›x2mPSR4FGL J2045.9-6835?éÇðôRÀA»>ÄaÀ:âØK%À<ö¥Nفç@ßé"ÃÏM?ü<cþ­©?Ë×î©ksÁ?èô¨H‰Î@uh¿ÜúA@"…£Ãi!?­t²ÄL¿àÞç+ž¿Àøÿ%:¿ãz›#¿îR£`—ÅY¿ïêÈ@ +šPSRpsr3FGL J2045.6-6838PSR J2045-68?̹«Ì³3?Æhm§DÊ?çŠÌï~Ë?ÈÖD£Q?«S<€xŠ?¥a˜Š¸¢?Õ&•ÛÉêÅ?È7ثʖ?áCóÀxù?È"+ñuy?À¤œyjF'?±ü¸6žA?ÒX+1‡?±÷r)ø}Ô?ã™l´ÍìK?´L@U$?¹Ôi¬Êw?£Ï5"oÃ<?ㄊSßã?­¹ojú}h?Ò[hÐã?«N¿Œ@—?ºn
xَ?™ó™Gí²ÿ?ÌY
[+Rr?ă‡åÎ6À?æƒy0ºÕK?Æà@ЈL?³2!ˆÖG?°¤d`Ã2?ÇH£ï­?Ä3	Ø	œ?åDÚJ8ÞC?ÊqÞÌv;?ãóÁ—H?º"ù`q?Æ°>ƒÀ·?®"c9œj?ça<Ÿ²Q?´L:¶Í@—?¹ìםúì	?¥±C(w?Öl_#Ñì?³'~e×7n?ÝX¾XÑäu?·Bg[=oK?É1ª">?«Á/¼"vMIXED4FGL J2047.3+1051?ì¹"Æ,0À3º­æW¸NÀ:K¼£n/À<8öí1Ç"@Tö.šó?û4+'»?Á†}]"ñ?ØθêÑÆ@£'üÇf[@¹ù$¹	¿îü¶¿š4I?½_e@KŸ'¿ÖEìuæ¿Û
b¿ù¿ëLóc9‹<¿å€Þý{ì5PSRPSR3FGL J2047.1+1054PSR J2047+1053?í?†ï"?§7¾D§ò? –c¤Ø š?™âD&w?«q-b
w'?Ÿ2M¥½MÛ?ï~zÜaŒ¯?'/ÊH
4ò?m¥SA‰¢Ø?w¢L¨–?ˆ÷ô ]k?‰RheÑ?ç?Ò®Á§ˆ?² TY)¯?ÅK1	jë?¬'êí©y&?»ôÔ#"jí?¤gÏöa–?íYÀèµX?‰ÇU>Ù?ÎbImí?nÎ~‹hÚ?°þ`)^¾¿?†¾.>«?êÉeŸA#a?·ÑâÉ(÷?²Oö±v?ªÙ'¶"©?·dÜRÅ­p?«ºƒw'é5?î|€ "!Ê?¤ˆíµ0Á?‡6rjå?"ž[>LéS?¢jYw+	ã?òøé1ó?äPÉáWjÂ?·Fä±×U?Ë^êǽ"?´{nÕ-–?Ã]í³™—c?©À…΂üÁ?êþ¢? ™DtÔ1?ß?¶¼N¬?…òg—è	?™'&¢?Ÿj&¶ä]VAGN4FGL J2051.0-0826?­½Š™À>cC,¥zÀ:š~dž;ïÀ<¿,Áÿê1@›™¡ýj@o	A=?Ä©h?ä¬(²¦°Ù@Ñ'o°'?ü÷WØYý¿ïÿøþÙå9?ïÿ¼]éÀ#¿ÊöˆÝߙ®¿áaÝøï¿ïÿÏ"èbU?ïõw`‰­"PSRPSR3FGL J2051.3-0828PSR J2051-0827?Ѝjƒ£Û?ÅkZ-ÀO?çlT{ú™±?Æ,¯$_¸?'™Ñ"T2?šÎÅAàm?Ó»àš£É?É)EÁ\?â=£¼ç?Êe
ä¾
Ë?¼Ž"œžu?±´¼­gÿ?Ѥ:KD;?±oDVÑ2?âü‰¿~R?´É¢TÎð[?ÁÚ­dk~B?©¡×ø•?áӘ–9gÖ?±0'ªMK+?Öç4:!ín?°s¡Ù^Iš?µÆje??šiõˆb3?Þ¾¾äy3?»|9UH?êV"jQ?¿6ڇ s?˜IwˆÆºC?Ÿ/Ýóý?Â[@zeï?Ã#}&yð?ç	g³Ô"~?Dz®"s}â?Á ¶G¾õ?¹Å²;Ñè@?ÄØaœc^°?­îòJ6F?æb®Ï›?µï†lsÏ?Áœã'Nšå?¬ž¶Ä4¾?ͽ•hBÅ´?°nú@‹?ä£	UÐ?·…Áéw…ü?Âޏ—ã?ª"Mñp2RMIXED4FGL J2052.7+1218¿ë·ÄaÀ3ýµc#»ÇÀ9äÂa8ÿüÀ<(2áԛÎ@>"«n@8Ÿƒ¾f?½–^%Ð;?ÃB'_ŽZ÷@ûšþôg@à?¸o?ﱿàÖ'¿án'xbè-¿âÝ6;ü/'¿æÓ\.§¿è0dxO¿ïíh]â^YPSRPSR3FGL J2052.7+1217PSR J2052+1218?ïVmȸô†?ƒ]	ïcÄ?eÇyíö?W•f¿‰¼?'mõ¸}?'>Ǎá9?îٍßôi@?$Ž/á£?†0ëŠÀ?"Ó¥ÏV?™¶:eEä?–r³'"r?îùí3l
?‹&ü,?zÓIaʨ?yí0!ŠY*?š
‡={ª~?…â/éâ
?ëóÖ5,ì?"q-îŒ?¥¨¹áÒ\H?}ªÄ†L Æ?µŒñdû?‡Uü±¢í?îTGSš?™0ð$û?€Û#¶Ã=?vW`sç
*?¦"ÅŽIlK?–…6c¨ìª?íbª¼y?°°©nƒ®?™Ï¹]¦›­?I'§)Rž?±ƒv'³Ï?©
Í´X€­?í‡.w⏭?Ÿî£t)k¶?€lŽ?†—Öõy)?°~ª¿—?›]1:]ê"?æqU0š7à?¢_xÝîP?¸Ó€Hº¯?–U¨C¤œ6?ÉÑþ…£æ?ž¿ TÎØNAGN4FGL J2055.8+2540¿‡ÐöDm×ÅÀ)
7.jwÀ7ªÃvõØÀ;¨ÿ°NçÅ@KüŽ0"Ø?ýpä8ú'?ž:öËù¾?âËt8Ùe@Al?Ä;.@ñœs)˜?ߓ~AÏXB¿«,F¯çº¿ÜÉ¥%	ó¿ê "àwN–¿ï z"Ԙ¿ïÿ atd+PSRPSR3FGL J2055.8+2539PSR J2055+2539?WѯE4Šõ?[ÿ'k²á€?ïÇÑô1ž;?ƒWÐ<)þ?v"š%±ó‰?>›¨†×(?^è­Mâ~?¨†''¼W?îl0Àœ¾?±cêÎ$?¡
Š‹—tè?§ÓŸxüw'?dƒ?Ž.xÍ?í› ó?¦‹/í…3n?²ê';ÝV?¥¢§úÏLV>šû%Iu€V>¥ÊöäŽêŠ?ïí4Ýñü÷?[¯x1αå?bÊJq'\~?[®,"ÿ?\ŸÕSŸ?Zú³¼Ð´?ï³PíáÍî?ƒåPIÂv?T†ù«Ë?©Ò)¦¼?;áÁr?•˜M¬?À^?ï19€K·?±'ŒôÛ±?–±O¯ýe?¯øúÙ¶¦?Œ{:VÉJ?ˆá
äóC?íJt ïVî?¤€£¸D¼?²ó¶p"é?£‡`úJÐ>s°‰=³ÅM>‰¹™¥.ýÝ?ïßK–›&P?m¿ú5v"Š?pZ!™¯?m¿Ô'ž?ÊPSR4FGL J2111.4+4606?îÛÊõé¿÷Dº)\ÜÀ7Ä 
a'ÒÀ;Zƒ®Ò@iÚקqI@#.£yè?ž¨e—çñI?а.[ˆ@,Q¾ôœõo@qÁcb%?ïÿ–¹‰$¿Í}÷<7ç¿àø¦Ú'Q¿ã@5z5PD¿ì¹Fk¿î<@".þñPSRPSR3FGL J2111.4+4605PSR J2111+4606?†y‰jÁÒ?†¾åd?ëR½è?¼ǗêÔ?À"vr?ºŸÈrJ^?L:¢/˜´?¡€
gžT?é‹z;IF	?¹b-e¡–ÿ?ÇýSjÈÏ?¹­!`Î?·?'f²W$?¤™ed…Q?èàÔéâî?°¬ºõ•?ÀßÛxÈNõ?¨'®Å-z?kýUBâ¿?Z_¢Á#"?î_—YX?"HÝï}ß?­ê18f‹Á?Žã·3®9V?~Á9·Qã?>`<_f?ìp…éä_»?´¥^‹s¬?º½üo?³»ë"§?€Ù°ÏWùâ?‰CMS&
?鹓|Ÿö?Âð@vpR?ÈˆÍ*?»;6Ú)#?¥zê͕? -8ß'ø?ê|v)–Á?°'Ú¥Ióa?À¯£žL©?«Mu'sø…?Jªv^ø??µÿ²š?î/ÏÑd?"Ò©wáw¥?®DÐZ'Ï?"­"ž¡§kPSR4FGL J2115.1+5449?æfùѽ¢b@{>—ÔÀ9«Ã½Y'CÀ<H:vôS$@ AjT‡–¸@S%A(Ï?ÀÞjÄoF?éyvCS;ç@ Yªu[Í@5euû…¿ä'pÀ²b=¿ßò([¾Âž¿j‹éÐ
;e¿Ü=eü‰(¿ìòª¬çT8¿ïÿÖ"î9PSRPSR3FGL J2114.9+5448PSR J2115+5448?Vp^æ)$?cºUìO?ïƒÁµ0gÁ?—à
Ê­ˆ›?ŒA†Éb~?–r÷u@>¢?'<E{kM"?žÌëNľs?é
p¯H5?Ã9²žxPŸ?ɄEŽChú?ÁîGlŒVv?®óŽýeDH?œø(³7q?éϲâ.͍?­®COåó?ÁP¸eú?¨6ÔÃàA?™ãïŠ.E!?''¤!Ò̍?íW'Jð¿?£_m$¥äœ?­"ã‹ÜëÉ?¡ù-ž‹Ö>?\½dËÃÏ®?g"òß?ïhaÊ®Q?šâi´RH?''ðwvá?˜²aUt?‡?š[¤á?‹TÿˆLDp?豂ïUŽ?È#ï¦ôÿy?Ì V2wݘ?Ç¿Ø#(_V?¡– 0…°Ž?—"ý‡´ý"?ën‡`m9P?¬BŒ	Úa?»ÀtàãÁA?¨% i	·l?k‡û*èêÅ?]C÷þ¡t?î†KòOpß?žÖF
Ïx-?¥âÁ&Œ—å?žVj±õ!PSR4FGL J2124.7-3358¿±•2BI0ÀF¸øa¦
EÀ7ú=ú	FÀ;Óc7ݼß@꓇0á?ùp0dKÙó?¡¥€­oÊ?àÿ‰kV@=÷Ú+Z!@)‹ê"n?ì0`†R•?Ĭ	É,"B¿ÐÆÚ¯ä^º¿ä>÷âz3"¿ï"NB_Ì¿ä±ÈcäPSRPSR3FGL J2124.7-3358PSR J2124-3358?"±³c;±?Ÿþ"/r?ìwsüPH?ĵ¯L¼Ï²?·$zɌàÕ?Âè 1ÁÍ?"'ݛ]0? ,'çA?íÌUÕ/Øò?²Ÿ¾¢—¸ý?©q¢>4ÂJ?¯Þ€%¼š?¡Âð®ºy?—l¤þX‰O?è˜ýŸÓo~?´ÈêÙSù?É+"Ć"i?´(µ%Z:[>Ø¥SêÍ>ÝŪ|Ÿý?ïÃ+ÓA[?qäã-_?~dM.Ìd$?qá¦8…¥?˜ÜCê
ðñ? ©Ì¦8Ü?ìð
)ðP?Ãü@?Fx?¹nœ-G?Á
‹În§A?ŒÆÿvw?•üjûõ¤õ?í̯ëˆe?º2‰·p¼x?¬Aeìg?¸ówsŠ•? J)m,kR?•õû,›?è}šVqÀ{?¸o^¾™‡?É÷L¥±;?·ß¯5Ì»f>¼X÷A>ËP¢Ú‹µë?ïZ¥VÕé?…sŠ@.Ü?Œ(sÝ4ˆz?…rçô³€&PSR4FGL J2129.8-0428?Î*¯ùNØMÀBz弇Û+À9»†ýX†À<WêpKÂ@PV¤&c?üûtëdg‰?¸+ƒ–%F?ÝN-?SR
@ 4)ˆ;£@)nÑnòý?ïøï]€¿²ê†qÏt¿×Â??°ï÷¿å•yyh¢¿ë·ù1~'¿ðPSRPSR3FGL J2129.6-0427PSR J2129-0429?¯Û8†•l?­Ái§e??ìvÚ)?¶¡¡Û‡z³?¦Meß8ýP?¤cMB®f?¼•âçkß?·a¹`6á?èÙôáZè?¼Ô¡©ο?¼šyq
¼à?²hd‹
ƒ¾?·"ÅÕ']i?¦ì¼1m7?è±hFª"B?±í¾·oÊ<?Áwûü²?ªÀÀó!`¨?Ó¾}Ñ^yT?¨í™öáž@?à7–Ù'H?­!%cx?Ǥ¨ù*p8? F¶v2Ý?žÔq$é?—o …lÍ?íµfSÆü~?©i™»lA?¥?b1÷"? ¶Y¬}?¬JE|ï'^?§'H'‹¥ˆ?ꋔ:VŠs?ºEʬk-?½~;oA×;?µßðC?¥'#ÛLM~?›Lc(¶†?êûH!ú4?­‡z•ðD?½d­f?©Îb®9?ÁéPÑ~¸B?¡¨‹ïŸÑ?ãfLP̲\?²™k
6–·?Ð>¾õ§?'?¬ÛòÂàPSR4FGL J2140.0+4716¿¢‹y~ÉPÀÌ~É3»À8X«m×sðÀ;ÈY±L=Æ@3xÁ1ãþ@}`ݐi?¨Gq¿Ç?ä¹V}»Â@2fz–¼?ûÃrƒU4¿ÐË+!–Ó—¿À¯HW‡¦R¿à}·³àm¿ëSž­ÕÁ¿ïÿr;†¾Ì¿ïÿ÷Âé±PSRPSR3FGL J2140.0+4715PSR J2139+4716?SOŒW9-?T°6ñ?ïS¦a9g?¡ .0?"V;ãŒq?¡|ÑÇ9cD?Š6äŠÜüì?¬àɯ¼Ç?ë ¡P¥½r?µþm" ‹?ÁÚtò4)?² ‰<00??:©Þ±æ?‹"h(çE?íž2ÒÝo?¡q–;ÞUö?®N(\3•U?Ÿ/ΈÉÆ?DÇ{i—?
ñéT¹…}?ï±üméy?r1«Bì=E?ƒP\]©Ìh?r.Ïx²?RfHëH'?XC¢Au?ïPþK[.`?™Ðà̖Ò?"¾À1ÃMp?˜Éç^+V?…+WŽà˜?¡/A¡Šÿ£?ëh÷:£Y?À¯g-®"?ÁémÓ~S?¾¶Yz®?‹ÑÌMçb§?ˆy'ç•>Û?íÒ¦òâO?L¨?ÈĊ?«ßbÐd?™¤|[!7(>è³¥r27>âˊÂcÝü?ï·Øª.Dê?sŒ+7âRš?'¨¾<¨?s‹P+'PSR4FGL J2205.5+6016¿ïö]?îz@
è<v©À:zD& }¹À;¼š*¹@"5ÜP£@¾mþ
?Þ
üÂÞ·[?ïýÖZHŒ@¹'m-*@äBtä¿ïÿÞ°ô)?ïÿó5bB¿ÞEÿÉú5¿â…¾'bE¿éû/¶¦ñ¿ëù¦_$ӟPSRPSRPSR J2205+6012?ÉàÙb÷	ü?ÂÛ(ºß9Œ?¦¬hßTžD?©ÊO_‡Ò?èv.í?Å?Í9H?ӟþ±îœ?Åxún?=?ĝ†Bú¦z?ºûðVI…?á	oè_?Ċû¸÷g?ã©JÐnþ÷?°Þ$ût&?¹¼äIJ™g?¥cÏ?:Iõ?Ò>1-õ[·?¯Åɛçh?Öð3>pÓþ?°ñOV à?ÍÙI¿´ò?¯ˆ«à?Ú#'áµ+	?±Txè1Ò?½ý_¼©?¹p¬¢ä/»?¹pK"Bi?·Þó£¢ÈG?é1ï–âk?ÄfÃclŒ?¾*8´b®Ý?¸V9-0?ÐÏgcé<?ÉP'´Íýy?ãÓ!Áµ†?ÈӎÓÃ?Ý[xÿŠ?²©«""‡Ú?ÂÀ'À‡D,?©ó*´•s?ٍ\C^`?²Ý,i¶3?Á)þ¼ÃÑ?ª±Ô_#4?җW.(÷	?¼ar˜›9N?âiÔç<S‡?¼†'ó\PMIXED4FGL J2208.1+4058¿­øí‹51À(/ëkôDáÀ:ÚøßzNÀ;÷։1@éÏç3€`@=r6~AN?Í&¢+8'ï?èÜsÔ
2î@
ç-@™Á1¹?èQpjÌ&µ¿ØTfB
g¿ì|º–¿åù`ß=虿8ˆÊ¿ïÿ5À+SÁPSRPSRPSR J2208+4056?ìè$ú?»è"t"ò?©­"UôÑ?ªíÑ=ðˆ?²â-ìMÅ?³>"&/Ë?à¦TÕ$4?ÎJÔ1'F?ÍîL%"Üh?ÆiÓ>£K?Ïxc‡'Ç?Å@ŸŠýÓ?çøĶ9¿?®¹¦)tîi?·Ãx^´?¢E~Ù1±"?Ä;1H)(?§7tD!Li?Ýê0ÓåùL?°£²Jâm?ÚV=¯
L?±÷<ºß?¾þEô3¡¡?""À‹Ï@?è›4¬ã€÷?ÃêÔÎ蟫?Â	q*?¢?¾¸˜ÖXÅG?·w—ÙSƒ?´¥tP+]ô?ÓA¶ÎޟÞ?Í¥BÉm
´?ÛL¶ø'¼?Î˄ǿ5¤?Ñr,z(Ýf?ÇÿJ6?ã7CVI–U?´‡YD³?Ã)ïÆ)£?­þ弜xÓ?ÏùâÕÅ?¯hØ4ù ¯?¾o{êä»?©€l³ó½?ç'|+ʉ&?¶Ìceÿ.?Â~Q‰ài?­œ3˜VûMIXED4FGL J2214.6+3000?ܨ&güF@À5¬9-Œ*À8)"UUÀ;Þ\Nµo¹@û—OgqS?úð.½§?£U$'ìG?ßmrÿÑÜ×@9ÔfõŸ@§]žk»?Ó˜ÂÚÄ¿»ã3–…h	¿Ö\²3¿äʵ€í ¿ïÿéYËMq¿ðPSRPSR3FGL J2214.6+3000PSR J2214+3000?uŸrÌ{CB?³œ¬¯Z?ï5ð	?*üG–©?cÝb-?šñæŽt4v?˜Iè¥r??¤-Ÿrçø#?í²6=Ô¡Ø?°|ötáµY?¨·§Ñ´ Ù?ª¸2êk¡Â?hYé?–aŽH)Oà?ìœÉC¢d?§
îÞ£¤?³Ô]¤pÄ+?£†¦{>	²?Ś"YáÅ?'ׯ4n?ïƒHäK·?{Îo?*q?Žö;É`®?{¨òËa¯G?v9娞	?¢n 4Ñ4?ï¢DH.lû?£÷OUžZ?x£öÓP0"?'±ŽÕ˼?'€Œ¹S¡§? xÌ´E?îÿxE¶î?³/+@êd?¥/ ²ŽC?±
CÕ)Ù?&'±õ±?´d©«h,?ílwˆ³Ôj?¤([Š\">?°¹¾õkþ?¢Íҁ"È>ý»à-ç«Ü?ÚÜë´t?ï= e??‹Kåûº6?˜WøÁE¥¿?‹Eåߺ²PSR4FGL J2215.6+5135?éN·¥-OÀ­6 ¥ýUÀ8̎eˆðÕÀ;þršQO~@kÛÎóB­@—‡B_ ?¦}	bvº?ÒÅ-¼PÓ­@#%">5ŵ@Wå¢0Áê¿·,£Þ'N_¿Ö§]CýÜ¿Ü-l…]¿ãý/5w±¿ìg ÉN=¿ëò¥Z'"PSRPSR3FGL J2215.6+5134PSR J2215+5135?{ð7hR ö?w6&â%Ò2?ïïa"?'†Èzf€?–
xWi?KÂ@ïÃÏ?¬›iCä¦ö?±\s …œè?ã>[ sN=?Å«§kÈ?ÕïܕÜd‰?ÄtVBp¬ª?¸Q§>³?¦]§S€*"?éoÜÞV¦Å?¯©îXT…?¼0dÉ«?¥Ê­ùýüR?Åܟï…D´?£
¦+¯MŽ?æ¨Ê-Oi?¥ù¼A*€?¿n¶};P?›úVꢕ?yø2À?o+N ÃÂ?îb(dß8ñ?Œ¨àØt*?¦¼uÒði?›³
õ;Iæ?—‡
+àÏ%?ž™KGö¢?å!Güv'4?Çښéƒoi?ÔDÿ49SÅ?Çb9E­?¡ŸÛWH?˜
.wó½¹?ëûu¹†?¦r܏3ø?·š'HîQ?¢IRj—?«ñkrà_?'§L>Í?éê:Ëáw?¦-™OΝ¨?ÁZÓ¸EΎ?£+V ¾öPSR4FGL J2229.0+6114?ïÉÊl}à@–Ü»WYƒÀ6þ"ÅõÀ:}E$Í>ã@ë
ò[ý'@h
"'r5?‰¥§Cü.9?ËçÂÇeYÌ@A[5Ÿôým?ÿ2̾_ Í¿¢T(÷(¿Øj¾[›¿âÓÄ"ïï¿åXåó€¿ì;E»Ëó‰¿îá['—PSRPSR3FGL J2229.0+6114PSR J2229+6114?k-*iºËš?pÒ"Þy•?ëZÛc'J?Ħùi
	Ô?Â+é"È?ÄOòßù?oµ¢ÔÍ?"Zcp4<ë?íù.ú‹Ä;?µ1
¤ɽ?®q¶0.š?´ÚÖņøÑ?´¦ô‰\é?¤a·^-C?ä Uét*þ?µo¸/÷?ѕ—Ià?³nMùM­>†™1Ž5">É"S<3?ïÔÝ!®¦q?k(.Û÷Z?u'AòðÎ6?k(ÿ<©?acñh£Ý‰?céSÕºé?í9¦®š?·c»›÷í¸?¶ü¨*Y"?¶ø­jÈ6?q"BìàzÁ?—»vÿŠ?îrzMpmž?´'ÿIíL?¦¥ÒÇi‰Ò?²ÒÊ·7¨ý?©O¥ÊHpÚ? Cˆ…"ã?å'¢Ö?¹¼ZéÏu?Қç!ŒÂœ?¶íé=ãé´>cJå0è
¾>vzRþË-?﯐† mž?ƒIsƒ?"ÙwB"6?ƒI¨â4-PSR4FGL J2234.7+0943?ä§sMlÀD8ªà"À9WÿÚ@SÀ<*øÞ£@ 2×àÔ@-»à~í?²üPý+?Ú=ë]†˜á@!@åæyF=@
£Àäâ?ÛÛ°•^¡v?'9jYåúp¿ÚîädC '¿ãf0€ÑK¸¿ëùd€LP¿ïÿò^VÍlPSRPSR3FGL J2234.8+0945PSR J2234+0944?ÈÌö¤rÌ·?Æ
<S˜X|?éeŠçWÆ?Ç×µæ	?‰ÍÛÜv‡?F
5x$?Îø™¯>š?ĽD×Óï‰?ãÚsj/~?Å4x†hS?Á˜¨i&p?³Ê]>À?Æ
jŸŽ®¸?°—RXǪ??çbSîOå'?³Š	Zá?¸Ò‹L«¨†?¥'Ÿ}ÅcÞ?à—p!"ê?°™Õ&(+ð?ÖÇô‹W·w?­ã»?À™(Ê=j?ž#Ϥ(Ïé?ÆïÛI=×?½cSÑ'>?éèÐàÝ?½íþÜЌ0?†ÎƒFoF?ÃªWã†ð?¿äé'ïö?¿Ý¬:}vÆ?ç'Â%™?ÇåÝ%F?ÃÄïY­?¾>ŠûØ9N?Ã\×
W6?²+š¤;?è¡wýù¦±?´êÿ^Ϭ?´½†cgö?¤Þï¿4?Íúmí¡â?ªt"â'|ò?â;¤Ì'¶?±Óùnwt?É#-?«)n­?OMIXED4FGL J2238.5+5903?ï0.úqÿ?Þm:åÚÀ7tKAFò-À:×¥œàv@ßùߪu	@øB0üø? mXaÚªJ?Ó£{X)b@1¶®::Žq@=ØïÅË&¿ÈçV¦Tèæ¿ÕZºá'׉¿âø¾eUð¿ç‹Ýž¬(¿íÏ@ãȒ¿ïÿ÷œ"/¥PSRPSR3FGL J2238.4+5903PSR J2238+5903?EQe¼£rn?D®
ébf?ïfìλÌ?›E-k$?'|ÿ0×v:??o¢<dç?€Ä§çö€ô?"·©täö"?ê'o"Oã÷?²ÞRϦ^?Äé÷pösu?³Jd…V9Ê?"1™vøÊ?«‡æee?íTª—¡Oy?¡ª•Í(´¡?°ŽjÜ)҅?Ÿ|3_%ª?@sÂB2x¶?4VrD|?íÏw"£@?"Ð^iÒ2'?±c[Ýrø ?"¿ž`¡Ø?T~þŽiþ_?P
Qi¥¾j?ïG¤ÛÛÍ5?º\­Œ
?•ÃtŸ¿A'?Žt†eŠ?s{n•DÚT?{ç¸tqà!?ëDR Íï¦?·'ŸuœQi?ÂRÜ	Åjr?·^þjKÑ?{øåÅœH?|Œ°Ø"?î'""OòB?"Pe´ióq?¤^Á,_ÎU?'	^ûuÙ?}ÉS!@þ?ÃÀ­¸g?íÍm"xºž?šÏ8€Ý²?±Ž³ïÀž"?šÉÍ2ܟPSR4FGL J2240.6+5833?ïiBuÄ¿¹äÖg3À9eNÀWs"À;'ÊÇ9@¢	ç4'@Yr|õ%?¼*Ë/¾´†?ԞG=×&@³q*Ç?ó÷Œo?Ñ6þï´®?ë·3ÞSÝοÝá'ÑÖ÷É¿åÀʀAXæ¿ì䥜[d¿ïÿ¼ä!}(PSRPSR3FGL J2240.9+5831PSR J2240+5832?©çí™í\?¥©ÏŠZ‰?æþ}mm?È7meÅ<ò?͌{ðˆ¶?Æç±PU¿
?¥±£A'–?­E¨qFë×?ހÌ%)|ž?ēù@7†?ÞÈÿw2Ö0?õ6¾?ÄÂH3d?§ËO†2Æ?ڄJýÕ-n?²ç`Ü­£8?ې琿Î?±´îÔqw`?°¢¨ßá,?ŒC4C–-?ç¨@ª®ÙŒ?§Îi	LèŽ?É
©IBœ»?¤ñ6f(þ?•¢¿æ6?Œ"7oÿ	?çtifÿq?ƕ"é†cS?Кõ\Áš?Æ@$ñ"š¸?ÃÛ3-Y?–˜˜—Úà]?Üî-
r?ʆêŽî^²?á±S¿"?Êg'Mï?´9ª¸Ô1?œ×vÒwå?ÜÌe(£¸,?¹è‡dÞ?Þ%0(ðAÐ?¸µ™zF	?'ºxyräw?v£áÊ¿?éÃa-mæ?ª™ø…›?Æ»,¨÷Ò×?©mq²Ï&MIXED4FGL J2241.7-5236¿ÑP‰ÀKw' ÿT	À8e½²}–.À;…ê&yçM@'´§«€@Ôœ¸2?¥W]bW?à¥Ç¥EŸG@6üa'?þr܎`ÖZ¿°±×þÚ,?£PAá̹,¿ØĤà¹)¿äƒÇ4ÝW_¿ïnàR»Ž·¿ïÿ»ËǔPSRPSR3FGL J2241.6-5237PSR J2241-5236?d˜Èô³?sàD½ŽT?ïºPÀ¯?¨J–C®?›u å³?¦y1BºÚ?™¢ò³¼/œ?£S©b±È?í&ÿ†–w?·bV`6x?°_G$Œ\?´'Œ©Ùô!?…1"ß4G?‡¯Ð;°?írí¥Vހ?£†ÁÓ?±ÂoáƒJõ?¢TN-Vò¢? Ç¸Xåœ?øc*t?ï	õLo?2è9Ù£G?ž²
Kš0?-
qÌ`?gÊ3	؞û?s¶†ql&‹?ïFbLfi?£ñx·M"ï?":wY¯?¡ÎOËó—?'MŠdæž?œ!û žæH?íofÊ[Ю?µähi³¾W?¯âÎ*•¶Ó?³Õ0èbüæ?'j¥viò?… ŠqÚú?í×t|dæ›?¢¹T#\•F?­îñødÝ? ÊJÚwbì>àLf'§c¢>á86
½Á?îø¯jµš?"cHîe·? t5ƒRW?"b¶¿«bUPSR4FGL J2256.8-1024¿ìlÉlù†ÀM#b¶®}VÀ9¥[n¼À<EÉGÝ@Ž%·õz@?ÿbîᵒ?µ¿'Ò€?ÔGÁSœà@éö©?)@k • ãû¿ÒEI€|'"¿Ó¶z¢Þg¿à*‰
ÖØ¿åEcKÿ²Ó¿ïÿ/àîAè¿ëw´!ZBÂPSRPSR3FGL J2256.7-1022PSR J2256-1024?ã
»"5?É="x1?×S'y>Û?Évl÷WÃi?£)±Q·¦Í?™"fÒßðÈ?Þ"SÞ4ºX?ÏÓe\Ò?Ømž%fä2?Ìê¢Ú¤Àƒ?ÂàøÈÂì?»î,ÃØ\x?×?П)Å?³ý5ñw¨¸?ßGõ[¦Ö?¶VÝÌW?ÂðtÓ^H?ª#¥7Ï?éÐØçŒ8?¡aîÙþ>?·2‹§ðGÇ?–à[m¢¥?ºF³÷ˆz?•LOœ,O?ÓöM¯`?ÀÇÀúÛJ?ä˜ó[NQ¿?Âh®Ägè5?­²¬–´?¡YǗdÓ?ÖÞ#%7â?ΒôTâ@¹?ÝûL3¯?ÏÁVÎ)*?Çé«R²2?Á`ë&Bú?Íì5Ëò?²$£I™ò?ã™? sµQ?µÉ@bÊQ?Ä{qû^Ê?¬bDZ– Ï?ãœÇ‡¤µ¾?­ÅC–'¸×?ÅV†æIÜ©?¨mê_5Ä?Ì6ZýI
Ý?¤ÿ˜¹æ9\MIXED4FGL J2302.7+4443¿îÌÅNkTÀ+ü"«%³À7ý#!m8À;ŸDÔE@§ó3üÝ?úæé¸?Ÿ7‰.<~a?ڔšCã…@9AÅ3?öŠ¸³:T?ÒCÛí㿦ašNË?.¿Ó$"ô÷ŽA¿áÓ{½™Á¿íFñVI¿ïÿ°"—©ÕPSRPSR3FGL J2302.7+4443PSR J2302+4442?\GŒ†ã•Û?eW=Sû?ï5[ê6•?¢¤W›nò+?—	ì˗Y?¡žýcpý>?•¬<€Ü*Û?¨îÍEÌ©?íà€´ãw?±¬€r0h
?§!à"gÌ#?«-͖ò?ˆè¾Ø³Ùã?‡,œEdq?ëõ'é§#?±.?áõÜ?Æ`2V?°Šs¬-B>óCû:/ïV>òM>™îÐ?ïÚHól?zå´®'°?‹ÿ½¼˜ßü?zîYŽ`†?`ú¦h£Ç4?_ÇP¶L¿ä?ï$춢?¡ô>Îk9?™CVî*?¡6¶ä?ˆËaŠ+	?™oâ7®r8?îuØCùT?«íünD?¢o£^»ãv?©Ëcgĺ?"Ìb™jY?ïš#¤—F?똙­F?±oažð?ÀPڇDÆ?±2»%³ØZ>Ó1mé¶B>×ó%Œ¹~o?ïTÏY]Ù?‰%sÝt"?•dḝó?‰$¥"S§PSR4FGL J2310.0-0555?êËß@åíÀLó5*"8	À9ñº
RiYÀ<ƒ6ª¶øO@bsN×(›?û_틉5ž?¾rø-}½?ãáKŒ]@!#{ñèæ@›ûcŽß?ïöý»'"?ÒýŽ`«fv¿ÓfF…öN¦¿ç<ù jn3¿í×ÆZÂÄ5¿ïÿøÞ£ŽæPSRPSR3FGL J2310.1-0557PSR J2310-0555?±›hWT6?³-
Ã0‰?ìñ´žúú?·ÃU"à³?›oifÃOî?˜M`§‡?À£iã.Ê?½øsæùì?èˆí0O‡?À¬¤Vi¡¸?ºµP2·&6?±õ0IJ¬?É:7q¹ß=?±Î¾$Ï~i?æ0™'iôˆ?³ÞèŒ;¥,?¼Å	<H?¦õÙºµ·Ì?Ú0{ÁJV?®¥ÿÍbñR?ÝôoËa_?±'ï†gX?ÁmÕ—? TÜvõ?¥o"T¹ªV?¤Ø_d)ûE?íתïµã…?°ªŸ%Ú·?š+yf¯r°?œ»ŒFù?´fjá(/?ºrqDïQ?êZç"ú"›?Àv¨nɌ?¸ÂXv+ø?²à™¶FŽà?¸'þC3Ó¹?§ªÛ֑-?é´¾æ&²i?°\Ó3[?º2
‹–™?¦ðË¢?ËÀ€,¥?­<Áÿγ«?âeÀ"?·XÆs·õµ?Ê«¥€Âù?­†õÆù˟PSR4FGL J2317.3+1433¿ï½È'Ã{ÀE;^Ès¬À;•'àÙìÀ=$)Ùî@¾CdÞØ@'#[NÛ/?؈•zѐ?ïÿ–ل@£ÃÙß@4ÛÐË´õ¿ïÑ	ro‰%?ïüٍ©Ì¿ÔóÉ[(Dÿì¾YÂi¢¿Ð×ͱÏ…¿ïÿM½øôsPSRPSRPSR J2317+1439?ë¤Dρ¢?½]¯Ù*?·–0Չ)¢?ºœþà†?¦'J«¡?£¨ï«|£?ìõöNåá?¹\:ÿµv?¦8÷ë¤øI?°	_lì?ªg£.A&©?¨V"Iç?é`Œ £þ?¯>¶Ã!Þ?¾<	=ó?©fgÃ&¿?¹W¿–™º?¢Â09ú9Ò?ëwU"kßø?¨`PÒ˜?µ¶è%Ú	j?£#Óñc—ð?­×kÖ®?›ÈØ´¡?çsìö°Bu?Ä«žšÆ{‹?Èà+æÛ
O?ñ/B7Ýè?² @}5Å;?©Ì¿Šê¶4?æooV¤ýP?Í©3úr;K?Ã¥'+èç
?ÆÅÀáSŽë?w]b9?¼ßÉûGo¼?æG\c5âî?²áݜê@?Å0ÇúfIF?°D×!±Íå?Á±ÆxÂ+?¦Ö"ϐª?âՀVã$?¿¥pÁ¢æä?Îó±NR?¿2ã	ؤz?Æ¥ü´%?·£wAGN4FGL J2339.6-0533?î<âmŒº'ÀO<Øý\·'À8Bj4Q@À;Ítj5(@à,Ä.B´?úê°¢¥²?£ÓցVÂ?ҝ)[™ñ@0í·'êy@é\‹{õ?ëVáŽ$ñ¿ÒÅ}Î¿Ö.ºJi¿á^n€[˜¿ìÂåÃ=Ø¿íˆdüPSRPSR3FGL J2339.6-0533PSR J2339-0533?©í}Á?±6¢?ìQ¡u†?ÀÔ»Äæ'?°|jDþró?µÿŽ9?ñð?¯:yq?º0lÄÏRc?ë–R˲y?Áµø(.?³²(©
ø3?±w|é?¨ÿ¥¡–'r?4L/Oñ&?ê[ÚbÑJO?°[ Õô?ÀP­ç>é?®Ÿ®ÐpB?‹KNï£ä?}‰ø¬A™?ë"&"Bd?¦"³"i§Þ?¿ö$ìÀÕj?¤át
Õ L?¡¦(·óç?¤ò·°ðs&?ìÔ¢h96?ºë
~ÍÕ$?°Ï§µªá?²Þu‹…JP?¥@¢¶½…¡?³nõ=D´.?ìQÆ{úÍ;?¿Uÿ™†?²ÑzÄ\ß×?´'óC­I'?¡ÿU³Eg?™"ZKŒ+®?êð¼tK<¦?¯PRqʚ.?¿zq†ç œ?¬N›{+?vœïÿÊ­?oÊ4ŽÌdß?êJµä['V?²oqtXå?Æ @î˜à?±«€q|PSR4FGL J0002.1+6721c?؎*±b@Â[T‹À9Ð'Ai
À;2ɪ@o£c@ëˆÊ>}?Ê©>þž?ÖmŽcZ˜R@¦÷ µí@S³Ü:ÿ?Ø3ºâ¿}Y¿æ­ݨ<J¿âžâ^.‰€¿éB"ßοïÿþ½à ¿?é§fN³OTHERunk1RXS J000209.4+672503)?ÚqOË;Ê~?ÂcBËè²m?ÄÙyeU3?·xÂt]?Û!󦑊é?ÂM"º‹?â²[Ô´?Ç¥{"ä?·	3r'°G?³-ž
š?Ö1‹¾9·?ÌeØ»²7?Üjæt#úl?°vÑ º!ß?­ùBK©ø?§OUoŒf?Ú>é£OÙ?°±4hÅïÁ?Øî‹Èdw?­Ô)Jl®×?¹U?7t‰?"ÛçË?~Ò?à^4étV?¬Td±mf?Ébã…æ?ºÈÅãñÎÜ?Î
õ¥ÍÉ?Á9¶@T•?â8ãü":µ?ÄàÁæ«?Ía—ú÷¿?żˆQGÆ=?Ë~š æÑ?ÃLëç«[Ÿ?áåz˜\?ÇÛÛúMt¹?ÏsQùÇú?°	šD¥¦Œ?Æѹ
Û¾`?®"âùB?ân½T.
?³t¦4?¾Q¦³*Ú? QbõÍßã?€êºã/)?¤;!ŽüúÀ?畐záó{?©¯¡«§\RMIXED4FGL J0002.7+7220?ï‡sRnH@#¨–»˜ÇãÀ:hã1" À;}¹?QN§@e	Àóû@H_ÐJ/Ï?Ð<ÌÄ¿78?²[¿ïCÅ'?çFùž¼ï	@HF6p)‰?î–ÿöÅě¿ÖOæ<Štä¿å	Ñ:×B¿ä"è™¿ï'Æ0ÑY$?âãA&
OTHERsppSNR G119.5+10.2?èX	'ª?Ëÿ‡vεÓ?i+ójǧP?d8¹skj?Î;)꽬&?ÌmTIáÔ?ëºgö<ƒ?»¡ͱò?‰yZ`aw?ŒùxŠ&ö>?¾ý•	ń7?¹Ð³ÈU*?é0þ32m¢?­Š
*\g8?•ilk"?ñ?Ó³ bß?Ȏ٦hκ?¬}`°Ù?ìŒuÄ?˜'¦¶XYB?}ùö¾õ1
?bµ‡ j?¾ÿ¬aâ?—}øJÌNo?ãõÄ9?ÃÀ}lsØ?€ÿÇËU?yëéŸJÆh?׌zù+¶£?ùá°/È?æ+Ó®úe?Ëys$v<?˜æµ¦÷mc?©-?þBœ¥?ÒíGÒ¸°?ÉéêõÌÉ?ãÇFþ—A?³uøžš‡?§)­?Â!s?˜TS4¡¨?Ռ<[GpÏ?±¤$Þî³?äáš­&%?°7áíÁ.?',ò"l?ƒúé°Õ?Î?Õ¡ÌæE?¯×U;¶¾AGN4FGL J0024.0-7204¿Ù€°á×ÀFr¾ß¤@À8Yø©ÊiÀ;òkón!F@y§¯†ì?ûäû,[¨?£g¿j?Öìþ{E›–@4¸Œ£è?ú"Ï»¼Ë?ހeëí#"¿¯kR3~‡š¿Úàr%uZ¿ä.b"óè¿íè«ð´2¢¿ë©;}"OTHERglc3FGL J0023.9-7203NGC 104?uzYQû'?{ƒ'F¨Ì?ïUxá¾!?–3±-@S?ûu7׶?'ï¬ËÊ?".¾Û½8?œ~+¯$S?î-­Å ˆ¡?­œ³§¾?£
Ę-°S?§Ì°ú·l?"âqV5j?'ñ~4úŽ?ìB—]er?ªÒ$¼­,å?¸²Àz¤£ó?§ûíVó_?Eƒý¯ÿp¾?>ÞéT
Rý?ïË&.'å?‡¹S
è"?œÚ{GZBÓ?†´Cl?zÒÍ;¸_ÿ?¸Z±¸Š?ïæv1Æ?žJìE4¨Ù?–.}ëQ?˜+(ïiX?Š,©´ÍZ?'¢C är£?îuæÐ?YB?«GVz¼Ýâ?¡úGÕè»|?¦¹2ÓFK"?‹0…DR3a?‡,	TYÌå?ìبÕe'?ªăð=?µÙºʍ?¨KÒ§žÝ?-ÍeÊ?+3NL'È?î¡oË¥8?•žy*ÍÙÉ?¥ËëÊj§&?•‡ÚM¿PSR4FGL J0025.3+6408?è4ˆ;"k?ö¿ã°> ÍÀ9Yº !ÞwÀ;'µ‹g§¯@ "CÆS`û@dŠ=Ü¡?³á_èE?ˆ´¼¾?sç?ÖH¿aÕ2?÷>ó/âò?ïÿjCj¸Û¿Ê˜†t"è¿Ü•qaEg¿åÏ2ؚ`i¿á"?Žò¿çàÌÞë]\OTHERsnr3FGL J0025.7+6404Tycho?àm"d¦??Å0«·†ó?j…¼ã½õ?a]¦ÊgÁR?ÞÌ@¯-ç?Å5!¬ÅgË?ÝiŒî\áÐ?Ì/Äsa÷?˜p~ôûà¤?–9lX#õ¬?à‡µ'ñ£?ÌJ"¡Q?åû	!*·?²m1Übí?š8=‡j°?'sÏø©´?ÒhÎiÉ·?±®S."¥?åÇ®xV†}?¦qÃu¶?²Š›©›¿?'¸ržÄV?ϛøJSì?£lÀwÈÇ+?ևjEKÂ)?Àõ[ùÈOÝ?{Àô‡ü?x³_¨±|?ä}S['îÃ?Á"rÜ•?ÍwàèžË™?Ȏs*š~?¡sõØû'?«Ëeáí?ç'†–:G?ɨ±Ú®ì?ßÜv1¤V¦?¶'(¬:"Ì?¤ÄãY¸o?–³½îHٟ?݊íc	(Œ?¶|‹bÍ?Û¹B÷vnœ?­!ÛrÝA?ÁFޘž"M?£Ö'rˆÒ…?Û£M»'f?®Ž)ŽÇðMIXED4FGL J0043.2+4114¿ÔõeêÕÌÀ5š¬§"W`À;
"ßþعÀ<fI¿f²½@-¤€¨[ÿ@0\"U?Õ'،°?æPràÈ,@M7 '½´?öؖVîú¿ÞDD}ˆkõ¿¬¸€‡qú¿×Ç
â@Ò¿îž/á5¿ïÿ¼þùoÃ?≲€ñ,(OTHERgal3FGL J0042.5+4117M 31?ìT)x|ñ÷?À^'I:¨ë?¡ú˜zµ©?µù¾ Óä?´a°pIö?¸hŸl:''?ëqQù5Ð?ÁSì?""?·n?rJ	?»Åº¬0A‰?ª{ýRè?§oº¶À^?åôC¹yo?²éñ&Y—1?¾S¾ª0|?ªó>l‡?Åq?4•«E?«ÇÑM?äþC&gÀ%?©…%ÌËÓ±?À)¶Á·^À?žÏkñ<Y'?ËÝ<¤© «?¤¼h¸'†š?éÎçH›q­?ÂÓ—›"í?¤É›<wx´?¨/ÈŁ)?Ñüõ/[?Áµ!p¤>?ãV…¦P??чr9E?Ñç·|G?ÐBÕLÎì?¿yôÝPí?¹§ÆÌ
b¸?à¥nÿÆ'?¹}ä=áõÄ?Ëz_~ô/?³-*PŸ?Ðø#¸@ùš?µ¤å,²È?×h¢s´$?¯ù±¾EÎÖ?ÆŖÓý©Ë?®Ä5gæ?Ý4'Žv÷?²/6ú=mMIXED4FGL J0047.3+6943¿ïõûÃ
@iìb"IÏÀ:ç¬è*÷%À<TBcQÞð@!BcMØ%?ÿ*'5Îîæ?Ê=£N¤(?¤0bp-?Þь"Þ ²?üë¯Ï;¿ïÿª¥Z—ü?ïø;`(^Ä¿åÑ3~²†¿Û"½'Æf¿Øþìɹ¿ãMòfºI=OTHERunk1RXS J004724.5+694222?ìÂ]ɉô?²ÚòNÛh?eI4£2 ?_™+-×ß?¹Bȹø?²¢°ùÅnÙ?è>«ö­4Æ?ÃÇoH̑?~'……½Ó?ƒø'Ðx€?λøFÖ²?Ãb¦¼‰?í{¼f£".?š'0ÔÀo?w"Â7§?y•{ÁÞ,?²¨Ð¦£­?™ïâäVÐH?í­—Ñ !;?¼áš?
ÔjU'?eog[ûÊ?°¡p—ɉ?2Þð(+?é1Ç,ÇG?À"åñԑ?w|–À׏3?s_6ßI­ò?Ê|þšòŠ?ÀZEæQÐ?ၫO¾H?É}±ËXr?‰n´Ke¹?•í–…Õ?Ü13À2ë?È°ºÓ%+‰?ê[ˁ.y÷?©q·Öe`?†VÊ÷¤?'ê®Ìo?Å'̚h©?¨y-I´?éÒ+T}ÁÞ?¤Åó=¨A?'ó^\ÜÊ?¢•¿Ž¤?ÆxæâˆÜï?¥G¥OîsAGN4FGL J0047.5-2517¿ït.VÁ•ÀUþ	þ†ƒ<À9¸×ï?¾\À<'~b¯@¿jë@,^,Ü?²zãáfaß?».Ï¡=|ã@	þÂé<@RÙâ)U?í8ÙÀ¦"ê¿Í]ª?¯…¿áÁVw¿ãú¯É†Ç/¿æ´EL:k6¿áágßjrOTHERsbg3FGL J0047.5-2516NGC 253?ïœÂ¦Æ?x"µsÅÇ?Vç?zûZ?K•AÎûkV?…òt¡ôy=?whtžèí?ï{Í0IôÁ?¢"\ÃëËÂ?u™gŸq?{3z‰?†ƒg>'»"?š1té¢J·?îçQë&¡w?"H·Œ›DÅ?…›ØÑ!w?"ÖêMŠN,?˜GÖ/+yœ?Œ…¶c^?B§øá?'BՕXÏG?}Ж¼õ@?cÕé­¸r?£Û‰LtK?€Õ‹$ÈI£?î¿ö~]9R?˜DKá	W³?p¼L1ëå3?c"é°N?¡é–®ž2?–çôu§.Õ?ï€"ýè?§	@',È?…šÜZv}'?A' ðP?"¯¡·­þA?œÏèÈxL?íRQnmØ?¢¢[n—‹˜?ž^5鑖¥?—žgíK´?«°_õ,>,?˜û&ës£?ìµ­‰Ä$?˜–óÉ|:'?ñ,{Ô¤Â?z=çR†ù?¶"n#®ŒÄ?—«š¼É
AGN4FGL J0058.0-7245e?éNÐà$9èÀF/Ne¾ ºÀ8f֕£jÔÀ;~ÚÉÒ+@<›=އà@üÅ2¤—ú?¥ª	ÜÖ7ã?·e~"é×@ò–pm@Pބ°(|?ïZ˜1º/¿Ü°žBö ¿ã1Í7U×£¿ãdâ¢÷ç-¿æí¾Ña‡¿ïÿDN
ª
OTHERGAL3FGL J0059.0-7242eSMC?ìÙ*åT?ª…:Z?'ž2 1Ðg?ŠM©[L?´ú€´ý?§™T—Š_e?æ~ØdÒßÙ?Êe¢Pø@?ÉÅÑJh?Çi
°ˆ›?¸3҇¥?¯¢¯¬{T§?éJÈ&b?¯‹þ\ n?µãQwmª?¤5þvŠmN?¿ÌFó¯e?¨3W0Ë=?ç}×6»±z?¢"7{‰'£?»‰@Ý0Ù?˜s=Ì?ÄD"|à.?Ÿ¬Ëº#
?åÜ©8Èô?À¹'Gë§?«=À0t?¡{òh"?ÒrŽ¬šl?¿Ø©
6 	?Þ]«<fg?Ð9 eÏ+?גbQȎh?ÐFdÚ0sÌ?Äääha?ºþ
~Öl*?å–éêD?±ìäšHì?»AàW¨·?¦Mú8E¦?Ì".JÁ?¬Ë/ì;Xð?ᮖüäË$?®—ã¸
g?Ç&Y³?ªRVËÿøg?Ñ¥,¨]4?­;k	:ÁAGN4FGL J0059.7-7210?ìäHRîÔ"ÀFwè¢ìÀ;$¡¯ À<pƒåÓ.@;uÒêóÿ@¯0¿»lR?Õ~aDh¶?ëc݊Š2@4	t@¼•Dj¿îÍ=ø:?åüO{пç£ôÑΔM¿íç	Ÿ&¿ïüÖë3À!?ã'‰|$TOTHERsfrNGC 346?î ñºöi1?§¡?¦ð*†?›96ìöïÓ?Ÿ{"l-Ô
? THÚùÜ?šÓAKäâ?ìêýã¬H"?¶"¡š¸á/?ªlýQ¡s³?¯GÔ`,?¦ã$qO?¢¾t`ÎA¯?ë/<Ñl™±?«[\$̜?²}¹ò³ú?¢åPMáq?´_z%ü? lAãùYá?ëS¡>öØ0?Ÿ«¬Å&a?´ˆâ–|r†?–"p³óí5?°Úr¨²õ?'@ù}+,?쫹Nµ‰?±{Ò1±@?¦e;~gVT?¥ÕZò·9Š?®ß3(aÎ?§­éáõAÐ?ææ|
C?ÌP9¾½•w?Ç•Ÿíy?ÇZf–7?ÀÉGuúÿ?ºµ8›8;?æö/ŸÞ_Ð?´–c®K
?Â6x·÷¨™?®=Kmš?å?ÁðÈȎØ(?©g"'ÅH?âÈØóÕ-?²d¢\òÛe?Ë×җð¸?²nÙø.?Éêeí?®Š[@ôAGN4FGL J0102.9-7051?ïýb¸ ´°ÀG¡ô±îÀ;@X|™À<Ȟƒ
f@ñà¬Óˆ(?ú¹_ÒÎn?ÙjCä'?éäNÿA"@uPÊï$@š6ù¼D?îð0Ä#¿íÝ.yÖ?Õç[ƒßH%¿æÐt!:k¿êÿsFT¿ï5?†'ÍOTHERglcNGC 362?ïÐ*
ag?rƒ u§?UilWMŽ?ZŽTp#?rª-WÀË?mIœ}bû?ït?ûòª?'_ÞNÕP?rcñ¬T++?\w™yl2?‰¾ErmÕ?†'`þÆù?îÝ^>q?žéu
­©? ºž]3óß?š¹ïd!HÂ?o!=?æ?'ÕSåøpS?þÿFi?"j§|M/?{Ñ+î±Ì?e~i 7? «jžÑ´5?'…Ö\m?ïl§
ùá¶?Œ¡N]?wÄÄ"1Õ?{ö"5kï?ˆóÛ7&ex?†hx±¹îE?îŠ^p×6;?ªSœRd.†?‡#…ã{²J?¦Þc¼?¡'7}K»? šÖÑûŽ@?ív"{ƒ•?£`uëh@? ï#…?šß®
pņ?§¯w§Vp¥?š8™jøz?íDn*;N?Ÿ×Š¯µ©‰?ØR$™?vükëri©?³¡Šä"ö"?žž<*M'AGN4FGL J0138.6+6821¿©Ënš2µ@ƒÅ¢6 MÀ9Á%q©ˆÀ;‡tߥíe@7fÛ¬8®@ú}ªOÊC?¿æùß)›°?³u67õdÆ?ó®K½m´9?íý°ðMZ?ïý'w>$ÿ¿ãþyC¿ë-Z˜¿çM	h^Ž+¿ä©,I4&x¿å¹^Æ^ô'OTHERunk87GB 013451.9+680621?ë>õéѕ^?¸}²Ø£ÓV?…SÒ²a^?‹µ\ÔÓg­?Á®ë-""¥?· ŸC
,?àËØCf?ÃÇî¶×m?±ÍÚ"|ªì?ªÑ8±G?Ùö_Æl¾ù?ÁgKyâ*h?çxýü*ï~?±%^	½Ç`?~­@P¹<?*ìñ8ª?Îl2gJ*à?¯âôkø ¹?ào¶Çk©?¥#¬"Jg?À`­ôÔ~?™X.%"s¡?Öñšv¾p?¢²º]p?äþ<XBX·?Äì/"Ž*â?¡JyIÓ?«øA‡å?ÓÚ8.´b7?Ľ´Qp?Êß8µ(@f?À'YÒ›?Àwÿ­0¿?½8žñ·Ì?å*2
£·?Â/^§ÖY?áÄ.1…?´˜Ÿ4u?«Ê=·È(?™éÑ ‹¿%?Ú|ªÀ³cð?³ã z©?Ì?"./Ø?¢'¹'@'>?Íkö¶¢‹?¬ÊÑ7º?á•Y>ÆËg?¬°í´ïNMIXED4FGL J0212.1+5321¿ï"ØÐnËmÀ…‰ïØjÀ8ÚÓC"LÀ<|ûÔ!U@Å0L£òŽ?ýàBæ.¢?«ØB÷¡aº?ؚÐÑ>K•@)0"»?ö­—}_§¿ÙÎ"Ë+b¿µèüoq¿Ü¨b_EµÂ¿åj	=ìIÀ¿îeÖS^Kæ¿ïõŠ@`B`OTHERbin3FGL J0212.1+53201SXPS J021210.6+532136?ujËç¡?z¦Œt¬ ?êÊÆ û;?Å8	ãò6?Ä)c"Uæ?ÄÁÀ""ñ?Œ"Ñ¿Ýc?š;¥Åi9?êÂõdŠ\ÿ?¹§8~ ÂB?Ã+Ý\¹î?¹˜—½=¼
?'BÍ9l"â?ðØv¢id?ë<úcÖ5¤?­^nŠ˜?Àã¼È¾?«ÌU?¸×Á?†š¦ƒ
ÆO?rúÂ]ØÅ?ìꨳùþD?œl‹ñÆ?µ×e<H'?šÿGµ¡?yj¿¸¦s?z8¦(É?éþ«¿"?Å8‹Ñs¿Y?Ç=HnólŽ?Ä«}ù]×?†žC'>1?ž2‡8Ygï?ë`s÷¸M?À,õ ?Á÷
=*?¾¯°­îv|?ˆÊj®¸—?ƒ…Na΃\?ìP*²'§?¬ùæ
û?¼$1fï4?«êV†°š?kçۊăl?^²' i?ì±Þ€Ïk?¡¨'–+U7?¹'ÐÝ´˜Ò?¡MvgwìPSR4FGL J0221.4+6241e?ÜòDŒ],<?ù—?·¥ôÀ8PÃí*:fÀ:ˆ ¼8*@ò§|Ü@@dß}©y?¹S;€""í?×|CG}m@d@y?ô†@Æï" ¿ã¸Û~@w¿¿¹Ó/<ƒ"ô¿áÃGb• Ž¿é@>aÔ¿í)Ãèø|~¿é+
oÆOTHERSNR3FGL J0224.0+6235HB 3?"š	\ôBu?›í1`!?è£ïÒq?Î3sþ6
?ÊÜÿŠdG}?Ío2ׇ€?'fës5iµ?žK†]Ÿ?âîw,Þ?ǔóU?Ù¢ïÈi*?ÇFÆCG?¸#¡ëƒ¹a?¦RÐa ¼ ?á3O@b¤?µ,$<0™?Öø°ægR ?³Ô¥€¤ø?' ϔŽ~?pM1â!?ÜwÆè:?ª×6åÈ°Ù?ág½Ã3_Ã?ªà]ý{G?‡y€ð6{–?ƒÕJÀ4ç?ê;‹"w=?Ɔ·–Òr?Ś;hi~|?Æ1&{óI?}D#‹?w±?ˆâ7ê"ae?ã˜ò"Ž¼é?ÌúÂëïÊ?ØY
i ¼?ÌÊ q=ôœ?©3î/x1£?š¨¨
!g?åI…¢'?·0|)J?ÒFx¡Á(?µtyÂ)Sã?qîDS'Ä?VèžM×#?à6ʅ°êª?³0¤O€?ßJ±äc?³.Z^MIXED4FGL J0222.4+6156e?¹Bä9d u?íõ,ÒÆáÑÀ6ã'[·¶»À:;`z"@½…TÖ@v¥xÊí?š±Œ¼ú?л0J@0}?À	oë@âFHä S?À›ïà"?¿Ó5"FK=ì¿ä°>Œ,ɍ¿è*¹¢"ª$¿ì틉5žG¿è=¦S¼?·OTHERsnr3FGL J0223.6+6204W 3?y¶އòj?y³ï
Û?r?é;Jû•¦à?Æn"£¶?ÊE#ë†M?Æ	W	Ú§ß?|…CHAžÄ?‡ÉMƚI;?êYÝÑyQG?´¯«ÓQ•?Å´^Ÿ{8Ž?µ;ù3Õ?¤®X‹ô2?t (ãzÃ?ã.wó½¹?¸ú\Ý?Ö/×ÿ/öh?¸a/Êyߋ?;}äÑDÍ?.G²cæ?ëMn¼˜š? è¼XÀž\?¾7Rý}ð? ß8ÎkC?p¹"JÒ7?iq›9‰?époîqÛ?¬çp"c?É¿$tÖÄ?ÂzU¨öPK?rǜC½y?Ý;ŠcQ?ë'ÑøÊpk?µ|Ïà?Á^{;ñ®ë?µ zD¥Þ?–ýÊ_xû-?'xç8$ø?äۘ™¶ÂA?½"Pž²?ÔØò&šëÌ?½0òÉ4Z?õ)3`?
ÝöÀ'ä¯?ë¡ÒÒÔ?¤\"›rÇ$?Áy°v'?¤[?¸D"PSR4FGL J0240.5+6113¿ê$â§Cj?ñfþÂ^§À5zÚÿ•wÀ:èâ­â@P'ԅRæ@0Ҁjôk?~>n-bÂK?ÂôæÇIÖ
@=[oâæê…@Vo"w¤¿ÀNÿYfú¿Þ‹É'—½¿äæMà^¿æŸŒAœƒ¿ë¨{Ÿ2µµ¿è,¿0|uOTHERHMB3FGL J0240.5+6113LSI +61 303?çÁ®d¤?ÃøÏًeé?µÙ,¶Õ/@?¶E>2"v?ÆùH'ûQ?ÀY³® læ?¥ÚZQu·"?ÂGåÛI[?ë
Ô;M€^?ÍX\˜1d§?¼¤0ûFÉ?Ää-7Vê"?ãDî¿ïL\?¶¸îtsb?É.s»Ž‹ô?°Ã {¦ ?ɽÑBŽ?°zJO™?"Âòáçð? ým‰Íºr?îËí\öaW?•ÖÅw'"O?£/j¥`-?•ÍUmK±$?Ù/t'#-­?Å¢:';ñ?Ë¿z°0›?Äç:TmH6?ØðÎĄÌ?Ɲ"Ïvå?«‡8úå'U?Ä'R®'hè?êéÿNÃ÷*?ÐeäËÇO?ºìi%Kƒ?ƕRém'²?â¦V7ço?µö̧Gc?Íh¦V/Pi?¶õ!ýF?ÊhÀPñÙ?±Î…"'ûŒ>øW
ýlË?yÕ*æxç?î:Efø™?©ábKº?¬[@ÄEˆ®?©
Ų¥yåMIXED4FGL J0242.6-0000¿è™ºî†ÀI÷%€ÃÿÀ9ÁN_¤À<Iʳ!@æG¤€@'šCㄟ?±ï¥ö,? : ×ùÒ?ë~‰¬¼Œ@Iύ¿âuác\ƪ¿ÝT»ÊàŽ¿çPÝ»1š¿æ?2Ȫ(¿ÒKÃãD2Š¿ïÿŝƒ‰OTHERsbg3FGL J0242.7-0001NGC 1068?ïÈÌÈ£¥ë?kSk=4ñ©?FÐn9áÐ?5?4fª7?x¿ßP+í?ió28Æ?ïì³~êc-?e~ÿ"''?1»Î+(n$?@¹¬"C»?aLÈ)(?bzHµ—LE?ïŒY#Õ»?0˜@u?bKJq@˜?hù´lÇ¿?ˆVäŒ]Ñ)?{˜ËVHU?ï͔ӌ.¢?UúÅÁ[M°?Hq¢¥?2××Æ£> ?v'aõ騲?TD6pÁgv?ïr¶ó¾öm?…eè÷ª…?[T­"C¶?Mº¥i:J?ç±X®_?"J¶bE§?±¼s?­\DӇe?ELàG
ö?WUbg;?|6"ÈD?€*­ú`ñ?ï77–?Â9,
Óg?u!!æCÔ?y»ÅG¥?š°Ç§¶9?ŒÙ"w:Íp?ï|ã6%?tm‰ìš?awýòÇxÉ?RÇÍ<;ù?Œq·…&–?ršÿ±¹¾ƒAGN4FGL J0328.6+5330?êÞįÙTÀ­È"#^À9øxG9zuÀ;£ãŸw)@ùqcÅwC@öVhÂa9?ÈBÎFIm?Öiü¾, @€_&×@
$àŠó?ï­Ä~Ÿ˜6¿¦=žàÅ¿åkB£é~´¿æ–akTâ°¿ïý®KØE§¿íþyzϪOTHERunkNVSS J032847+532859	?ÏwGù؍d?ºæ.ȕZ›?¨=#"»ý?œ	æCýl
?æ¡J/—'?¼¾–uš-`?Õþ=ûºò?ÃWMaæ,£?¶hâ'ÕÜË?ªÎl*gá?â3Ä°(~?ÂÅ*¯}\?Ú5¥Ä!"?³P åM?´"Y­½µ?šôŽz< ?àRÌ¥¬ï¯?´"ÂV4¿?ۗ÷üY
?¡À¥©©?˅>!
?Ðm;"Ýÿ?Ö¥hÿ6Æ*?¢BÓQ1‡?¾ùÕ÷÷Q?¬H\ŒØ?±ìœ»G?§è€.ÿëà?éðM-ì]?´–ë*M3ú?¾—ˆê—/~?µÕ÷A£5?¼ghÄåw¾?´k@›ÓØ?è !Êk?½žÅy,¢Ü?ÈI668?¬|ø•{Èe?·÷
|\|@? Á
´uð?æîÑ/™0ú?±¹IC]%?ÆúTÿOš·?ŸŒjÍwn?Ô¿¤ä.ù?«;n';]m?ßÃ0<øj?¬|eK÷3ÚMIXED4FGL J0359.7+4445¿ëkÚé'w´À0=µm5À:P "ˆÞ`À;æÝî]@M@H¯å`l|@È!å-ã?»ú# Ä¿©Œסçò?ïùÓ`dĦ?þ"EÇ	"¿êf"¿˜?¿'X¡p—\¿ìÏÀÒÆӿטh û£$¿ë^>¿ƒc!?áÏÐÝӅNOTHERunk1RXS J040006.3+444512?æâ-[¥9­?ÀB˜ÁWx¸?"˝€a—Ó?‹ß
}RLd?Ðþëp¯s(?ÀËè~â'?éåýd3?»jìêÆÕ3?r¡ùŒçy?t?ë"±Yw?ÉcX?P&?»¢ó=-?鼇v½ˆ?«>èU
ë¹?žœ)Iƒ	h?'oJ¸ r…?Å<¸ô¨´?©7Œƒ7€À?íÑ L¢V=?ŠØx|"yo?€ó¡ŠÈ-?eÄÉDkc?®©òñ°¤?ˆóáŠáJ?àÍ-
 Ç?ć€|è?¦ÌCeàx‰?œKÎydØ?یk9E,@?Äx¿y¨¤?áHk(d?É¢†þ‰ ?$[»ÒÓq?F(źÄ?Üæœ-?É ²æO]i?䫎›†%@?µNg]ÁD?«Þ•Ÿ…É?›Æ¬å\p?Ó-Ä.æ?³Æ¦übÿ?éj\7ÁëÑ?§ÝÑ÷øØ?œJnڝ(?†Œ	W${¡?ÆÍ>óÁêW?¦šϞÑKAGN4FGL J0402.5+5402¿ßfš6U/:?ðƒ
%ó¯À:ÔüøÀ;ñ4ØNá@"7ÑÌ?ÿx¹º¡Q?ÊÜ@Þ¡,?‹`Ŭ`àY?¾Ó¯êéÃ@›ØÚ¢"?ÔµŒßvó|?î<xVRó?›PÇåÿ›#¿æ—œ~ÑAQ¿Û0cu^P¿Õ×Ýašy¾OTHERunkTXS 0358+539?ìCÒùÈÀ?µ&¶¤x?bù·€þ×?a®«â¹ù?¾Î¯ñ[?´Ô£¯Üp?Ú%]šî`ú?Ðä%…ôó?"Ás«²ñ??f=
áò?âšKcçÂ-?Уñ¦á´?ìnn¦?¡Z<	ç"?€',V*"?xJ$'H?º‡¥ü(…? YñöÃdp?ì"Z({°a?—ԟʣ6?qW8¯t¦^?]YÁ1w#?ºÇ»3$ù?—z/hÉÒ?çH7ß ?ÀKÕҖ!?p®–ú'‡?b Žà•òê?Ñ-C5šý®?¿×tõº²?ÕÎÇù©NÃ?Ìï·ê^û?€æS;?˜×óreê?äÕ¶h²F?̙žYd?çžc›}A?°1 î¾ã?èœÄŒÛ?‡%ÿ?Ï©èj¯n?¯Ñ,ywé…?ç!;=æ?°‹B鴏?€"ß‹5f¶?v72…߬?Ñ8ꇝà?°«Þ߁¬ÔMIXED4FGL J0427.2+5533e?ë5ºOFº@P;£D=GÀ7éè¢ì(³À:Ìûƒ¶@"JjꯋÉ?ùV~AN~é?§þÅdÆ?´Æ´"×j¶@Á`@Q{Œ=e'¿ïÿòɶ—×?ïþÀ//˜t?ÔHk^rÒ¿Æ­ò2ql¿Ôàœbvª¿Õ¥µLOTHERSNR3FGL J0425.8+5600SNR G150.3+04.5?Ë:¡!ß_?ÂÙš€®? Æ('Qü?¡ŽÿUÃÓj?è$õ."'Ž?Ä ú$ã~?ã:ù'&O9?ЦµX^]?®Ù½Rßµƒ?·'½tۘC?Õ®ÕQ;íþ?ÌÐ9Xnà?ØSÚ5s²Þ?´
m
äB\?´ÿ¸R<ß?£>T|îô?á6ã`b?³©Ï¯-¿&?ÕíÌ茭?­Íî³¼?´ÑFµð2?™;Òoø+7?ânðµNØ?±¨!÷<?ËØ㳐ˆ?Ä6¹¶^e?©Îbк?©)˓WYZ?çwîQ-Î?şð´Eü?Ö\X¨¹?ÏÇdýty=?ÂëÅÞØ#?ÈN	­þ«l?à:#åú?Ï3sӌZ?Óíxpv'
?³ïÊieÃ?´òDž«Ÿ,?¦žC+¹¿?ãjê×FDÕ?³ÿC*!<?ËBt³tûÄ?¯¦ÇÞ4?¹™»ŠQŸ|?¨Bý€'†?åü+a؍?µÿîõ,¨MIXED4FGL J0427.8-6704¿ìµ¹×ýÑÀCFž<–‰DÀ9{"ÆäÀ<XÚ")@·«N!÷@þxük 
?¬e BÖr?"~­Úï$f?äsÂÚۃI@ïÒ#ù¯Y¿äÂB…5´¿Þ
÷9‡á¿æêL¼ƒ©¿äy'EÖ¤¿ãà>>T#™¿ê˜iñŽOTHERLMB3FGL J0427.9-67041SXPS J042749.2-670434?ïÈwT9,
?qõ£ˆkV?JƒXd'?; ŽLõÏ?xsêМNÐ?pöÖÏò©{?ïÅ@S­&>?€éh"èÎ[?Skn²?dF¿¿‹?x"ú€X7Ì?yd"̆?îúTn[@?'s±Ñ¿gï?rqY|z§J?sÞÌû?œ܉Á%?Ìæ55ˆ?ï Î;Èê?hÐE)	KŸ?pldÓLlb?VèTQì?´-»š`?b¦¥¨f«?ï]Å_'"?‰ÖÁA)X?a´Bdðï¾?SÏ$Êã?'ËÀmI?ˆ†°mL‡ä?ïCfâb5T?›Õ´ÃdÅÝ?e8;ÅýÊv?~Êþ•21?"ì8éØ+?˜×ÔVµL?íIcà
}n?£}»n_ìë?‡?pS0Eñ?ƒóòEÓ¯?²ÌòöýÙÒ?¢
ù;¸Ž?ïµR ¢ý?"Mã8Ö?†BXø¼*B?t}£>ôÓ?"È)6ö…Z?"V3ÛÜAGN4FGL J0452.9+5117?Ý»•0Ã=@…‹W"<À9Ò¨Žÿâ¤À;m0•Ê@@ŹE˜›@¸PXÝç§?ÇZSÑä?Ö¥¯Q'Ã@é.Àë­@ݜ²üÂ?ÎK™›òå:¿ÔUäswÇ¿ç-v% Jù¿ëð\>D^T¿ìí8™¤¿ïßøÞ£ŽæOTHERsppSNR G156.2+05.7?äeÖwV´Ô?Éõºõ½dƒ?žãø±ÜU?¯x­$÷í?ÕF"0µ?È!ÂÆAK?ä쐚þ"¼?ÃAÍ}ªXa?­NB³?¦2f1FÐÈ?Ò}z¯f?À·*.Šy?èO=3"}j?°Qnõ—?¦QhE—Aƒ?—)"Ý¡?É.± ýY:?­è…ý8?çÿaR¼v¥?˜é"À#+?«'§î­­?tõ¨"°e?É!ÐÓJH?•¶<ëØP›?×eß,˜1?ÀšÍ©Ê?¤E_a¯C?žøÑÙ;£?ã	š5\?ۏàT¶]?ÚW"hå?ÈÿP5U*?»5%É	Á?¶à"àtë?ÞÛ±	UqÕ?È?)ÃjDå?᫝Š~†?µ­óƒDîr?²>8!^?ŸÜÜÿ
Ö?Ø6å;ÐÞ?µ'4>ñ¹^?ÝóRÃs#?§&ÒHß?¾t‰¡¡GZ?˜ÿúfk¢?ÚoŠÓiZH?¥îN
{¹GMIXED4FGL J0500.3+4639e¿ï¦,Zãº@‡?i¢[À8:œÄÞÂÀ:ÊØ£š¤@ïCÿ‰8@:–¹ëH¹?±®+L	?Å2évј@k˽Ù@ÒFö^—¿£—ìÆ<e¿Ôä±z¶Õj¿æ×2ƒ2¥¿ä€µ¿ë%F Û¿éøDŸÂ'­OTHERSNR2FGL J0503.2+4643HB 9?²Ñ‹ª®ïá?¤SÝ?ê.e?ÊØ2ÄÖç¶?ÁƒT¤®0ç?æïÁÙK,Æ?Áü9V¸É`?Ñ(J™M¼?ÐR'è?ÙWjÉç.?˃¤3jTv?Õ£lë"3?Å-´ùÇVÁ?×Y%ٌ‡?´èK>AÚ?ɽÌÿ¢?®GiwÈ †?Üû?ô.2?µ)©™,f"?Ós~¶y?«ÆٶȲ?Àî.áӉ?™ñCó¡'.?â
µ=d?±¶
ÚÍ·?¡íÉÑؕÒ?—(xr—?ʟ¬qý7=?¿ð/½Ýƚ?è98F~¥´?ÀÛ—©¡Ç?½ÒD w?Å^YdU?ÜòN?ÏÉêÜϛ¬?Üum̉à?Ím¹p=n?к³«Ï¸?¯ýN¢^ëò?ÏÈpöÑòÀ?´•Áèî?à†hu›t?µr6¥VÜÉ?Â68KK?¤~~o£z9?Æҝ¢£ê'?®ã+Ð;·Ô?å½Ê""DÚ?·\))L³MIXED4FGL J0517.9+5030¿Õ*Kƒ8@NÏ~Wô´À;í$[)À<uŽÀøƒ4@×̃%äÁ?úÒ
#opÑ?ærÙ;p—?ç©8¨½ùË@;šÅ都?þGÙbÝDê¿ïüD=é?ïþašNË?¿ãÇ}Øró¿Ñ}Nñݨ¿ìÄÝëAú¿º_Êø®OTHERsppSNR G159.6+07.3?ì§Fš2
?°áIz€ b?—e fñ?'žìØc­?¹©}°b'x?®ËìœÒ?äïÁkÅ ß?Èú`¥ö?¯õT¼i?²'¶{%?Ò!ҐäœÖ?Äøå¸Î
?ìA'ÖèÁ?¥(|þ†ÂÍ?£Œ}³QT?•þïJ*d?µ×-2oP? ãÌ·‹ïx?êÞ""0|}? ¦|VYÛ?¥lL
mâÊ?–YØ鄡?¾XÅd´Æ­?š«øÞüä½?é'ŒsÁBÖ?·.1ê?ª1úlìb?¡Cå¥9Iž?ÄÕO"àÑ?µ"fˆOc?ÛȈìÀ?ϘPÄ=²?¼°ØiQìö?¿
VR6??ÝAᐘ?̙´á7»?émºv;¤$?¬8§g<Ä?ªŠçbðÓ!?›=|›»¡?æ\Nú'é?¨¢½¹^'?æx8מH?´ÚQc­ ù?§¸üÁt8"?©×f]üõ?Ðn·ÔÔ>?³3ϐLMIXED4FGL J0519.9-6845e¿ïñ¶°À@±'¡ ÏÀ6îñ<îØÀ:\pšœÎØ@C¡lv˹@Z5þ¿Ž ?˜Óy—ϼ?ż°µj¬@,H2ËŸ@5ëq…¿À²ŒÙÔG¿ÒÄË¡~•\¿âóó¢y'¿äªúêíID¿êWºÁÝZ¿ÎH"•sOTHERGAL3FGL J0526.6-6825eLMC?³‰5Ï«à?º|ûBð?ǯ§ÅMÉÚ?Æ®FS:S}?ç¢ïTûÉ©?Ƚ*¥<‡g?¥B&§Dä?¨ §Ñ{ïK?ì´oe_ø†?²£MÁa±6?¯œÇé–È?ª5i1?Êïûbë?®"kÒZ?Ԍ֡¦'?´Ì…$þ£E?Þh1ÓÈÐ¥?µßæǗ%B?x߃N¤·?gA %¨DÓ?à÷701ºÒ?·åؚ2=?ݱ!nSŠ?·Ìýìv؜?£Š-æ¤,?°cçΡ\]?ÓõÊQ¶?È%Çû'?äÓ2MkSò?ÈÈg³ÿ‡›?›l"_ç?¥•[3'Ù°?ìªÃȗ3
?ÀpÀk"LD?³ÎÚ'Ÿ?¾+g+Æ?ÄÄÒ»NJ?¬ƒ˜wè»?،¹vÙ¦$?º—=É?Ý= Û"u?·VL?Z6¬Ð>H?Pžyao£}?àx€Z`ý$?¼5!}†Ç?ÞôȞΫ?¼¼·š¥LMIXED4FGL J0521.2+1637?Þ¥©ª*WåÀ&©O‡À:–E"I$À<!]×MY@ëÉa2tò?ø~Ûrýœ?؃b¯É?ïNH,¿{«?ÿú"5¬Š7@ŒÕ»Þ¾?êfÆ"Ž A¿èðaՈ¿Õ@˜Á­^ó¿àåQÉ oâ¿é*‹"ÞQ¿â9¾'‡.]OTHERcss3C 138?ï
'P–Š4?šÍïÊnFÜ?^'«ò‹E?VZ)?œf›0É?šp¾ÈÁê
?îçÇürE±?¯ 8ڒ?sdSªHª?•àgà'?ž-ÿ•í¯?¬€û€#á?íAÕ0"¾Q?£L(²Ýª™?–œ
)}?Ÿ[|1çŸ?°JSðžâO? S¶nÑ?îzƒ¢È}™?‹¹ša^¢?q:;ÓÔG§?\øõP¢Ðg?¦0~[§Où?ŠµJhó£??î‰ ¨A'=?¥k–€?n#cë#ô?hN#fCü?¥‹¿GpZp?¤Ð8^¡`?íÊC@؞x?½¨¯iÃ?‹æS?©\@7+$?¬bã*´?·ï!˜-?ë"Ë"ÆÿŒ?¨""w9?  R™-a?•'¬‡ªPC?»QzWEGn?¤äŸ]p!?ìF¸³æ!?©L̐«£ ?€gòsu¦Ÿ?vÀꬶ˼?»½<µ5?¨xzÈŗAGN4FGL J0523.3-2527¿ÚÛL
ìõÀ=Ô2‡;ÉÀ9$éºC]MÀ<4x'@>^çÁð¦?ú[™hò1á?±
Á$"8?ÛE"~°	@)
fðÏáT?÷¡º¢¨¶î¿Í÷Pƒûø‰?£Drö—¡r¿ÔB©Þ5Tö¿âo9©nù³¿í隁öæ¿ïÿó5bBOTHERbin3FGL J0523.3-2528CRTS J052316.9-252737?™"ï!À?›ù•ÝÁIˆ?íì*¹Î(©?°#ÐøR"?¤u‰ìhΕ?¦Òmp?£I&‡Ð¯¶?¥Ýd
Á?í¶DäÐ>?°Ç>y­µ?¬›u(*~t?¨)Ƅ֋_?¤lˆøä75?š¶KÇwÏû?ëßD…ãP¿?ªƒSëά?¶Ï—S—wn?¥{äÝ!Ê#?šTÄ,´ Ö?…xÎ%š÷Æ?ë¦
Ø}&"?£=`̈);?¼:`4Y_(? nÁÞ?»¼mÔÐÅ?ŽbùaÃÖ?îe>@¶??¦z´&7Í!?¡N=¹i°­? Ò ™N?•èBÏ&|?—#
ÿ´ìá?틑TëX˜?³]	è®?¬RÉHÛQz?°ÂÿnŠ¢0?™—dÓAŘ?"# ãDz~?ìõ¡Áœ`?¦BÜâÂÎ?±íÃV'š?¢ÎÒ#s¨?…R¾!?vI)®hø?ëÑãYx?«oû¹¼}?ÂS˜¨œ±?ª?y;Ðò"PSR4FGL J0524.4-2413?çø‹ ˜Í}À=3ÚÄç%À:©VI¸±À<:Ȇìî«@R`¤.É@`Eºõ4?Àuf3¦¿´ì×?}ªŒ?íB–%œr@¯p¢)‹¿Õ|qÀŒ¢¿èÒ±þ•FÏ¿äö©Àd¿êáÏ=jn´¿Üz¡Ü´ "¿ïÿ⾦™\OTHERglcNGC 1904?ïèC@¾Ù?v†©Ù«ù?>Àõ0ÚÜ?0H
Il\?dž(|Ò`?veB—"·y?ïÒ}"'ƒ1?räϬ‰ãÿ?DFðÄz?QkÑØúÖi?t8WŒ½=è?oJ¾üê˵?ïr	™u¡1?{R²»ÉÈ?bž1¨Gs
?X²Køj/?ŽÖ
;}
?zÜúëæ½?ï¿eŽ$E…?\[Žù,ÿ?F¾q}ŸèK?4X{ÜӚ&?}uj²Ãí?ZÀû9EÃ?ïÑwˆf…4?qcËúeq?P®ŠÁ¶U~?EC¶ªÃþ?s™â´É?p-Õ¯?ïtiå)˜ˆ?³+™"nÀ?S	`ñ'l?a¤OPX[®?B-]AŠË?'ÁԚMS?îâgY3*­?‹š»çÿ?u3¦/0–?s"ý©¹d?žf+O†rm?‡›[¶k(Æ?ï.jK£AŽ?"êü?c8Ü"_ï?Y`àt…G,?—Ë›¹ßF?~JÔ«»ŸœAGN4FGL J0524.7+4824¿Ú£èPû‰è@6D#EfÀ;š%FáeáÀ=G'u¦@ úèóžó¡?ý}ÒÉfÿ?ÛD^ÞÜ?ï¦jÍÔ3É@s''%Î@Ÿµ§ís¿éÆl`{jÚ¿ïÿâ¾÷!?ïþFŒ¬KM¿}87Sÿ0¢¿ì=˨	žå¿ïÿúâôOTHERsppSNR G159.6+07.3?é–[¥%®?É&›H#þ?—†7
ɜ`?›:Ð[X³y?Ƶ̞1a?Çèã´/Œ?â¶é¥íÝ5?͈0Tug?¹^–>×gl?¿ø|¤§zê?Ô:‡#äû\?ÆÁ†ÛÚdn?ë;°7ôA?©™à¸ÓJß?¤"ë•÷?—•yBnáö?½D,³Dîû?¦ãÏÂ8?ìŸãMu\V?¡F.U±jú?¬Z-¢?œ%üÃÿV‰?©§È	Þ>ÿ?"æxÈÓ=á?ç4P.
%û?ÆÔݒlԕ?¤æ']«¦?ŸÂú-‹"?Íõ=#¡ð«?ÆDß~¼YÉ?ØÕ¥Ô:X?Ñ6¹púi?Æ°éÕ¤ÀG?Ë®,Àbl?ÛÑåBC?Ï×>ã'?è÷XȐt?­h±°ûA?ª6_šfÀv?›×¢ŸÄÚO?ŕö·VîÏ?ªºíF&ñU?æ€C9ï?¾Ýœ +¦n?«_J®F?»´¾–±»?ÂJŸå§ÓÞ?²º›?2±2MIXED4FGL J0524.8-6938¿è_†³bîbÀ@f>lLYuÀ:¯wOµóÀ<>¼(@ P&'º'.@#\ƪsÜ?Ƌ«Dfâ7¿q;ÞPÎg?»7…RdѼ@sÎáÏé7?îF7òµ•¿çM|5Om¿ëøýbô´¿×̤½äý¿Î±ZÖeQé¿ãòEÍiª¿OTHERsnr3FGL J0524.5-6937LMC SNR N 132D?ïdP´ÎS`?…IºÀ"õ?SKOP¡‹\?Foס—g·?'A4jÐ4_?"ûyø-h?ïÈ(á?†–‰6ž?_¯÷Þ*8ª?g`£¯(V?"—÷yP?ƒ"²§¤?îµ µÂš?"ªã'
Ç?j*ù"Ã?g¼©èëí?£ÆbÉz'?"C
{4ýÙ?îjãm<?":õ'Á†d?W2ÙUK'ó?A±#Zllï?¨žx¨<²~?"°
ûžx?î|ÄY5ÑH?›ÇÍéÀ>?jZýÁ?aı³1i?¦ŽP/Zp?š‹œYQ$í?[~'?žƒ6¦'A	?dó¦žAv{?qrܶ
ÓÃ?šMõx´éù?œì'úhóQ?í^~ŽXüN? 3UrU©?woßÉÅ)—?s\r{VeM?³•
'ÁŒs?Ÿ0Wqè
ý?곸ÿnx?£5Y²?s}}«Ž?ff©ìé?ĕ0^‡?£Ձ-:kAGN4FGL J0526.7+4254¿î_õç€á@<"Þ ²'À9¶5•
BßÀ;‰Ì·ÔD@r§qsŠ¼@'»0Ã?À=̀{æU?ÎÎ81ʨ@	Š]ò#žk?ûR-ÝZ¿ã>|b&:ҿфîê3¿çžfB)EI¿æ'¿BJ¨E¿ïþ&@Üi"¿ïÿ‡ÕK÷OOTHERsnr3FGL J0526.0+4253SNR G166.0+04.3?څýVµø?ÁÉÙN °‹?±¯WŽ4Ë4?¦?AÍ>‡†?à‡rŽ¾?Â?DRY-?ØÁ "	·º?ƲN·o1?ȌV
Ê?½n­æ5\?Úø4\܂€?°¶Ôñg?ãåͲ®q ?°ÍÌÙMhÝ?»1÷ÉЙ?£ÁǾK?Ñq˜°©š?­¡<¢³ù¶?á~®îò‰?¬<æb]?¾Â6™¢±?–PH÷þoU?ÕR"P{²B?«Y–ÏXÐù?Ãå]3Ú‰?µ½kÚkã?ÁðJ©$.¼?·ÃO5­?抖Àmï?Àòğ³?ÇýPOp"?ÂÁ6k¡ä—?Ю›"I›?ÃÃz¸W†?áñTž	bL?Ç9wk­‰L?ÙŸï7õ?°òㇰUK?Æ@' V?«p̑€ªç?Ûå?ý=zV?²/'T?ÒâØÌN;'?¬Rw=›Ž^?ɞ
–/p ?¬ô$ÅîH?à'4M?´+¿¼âØMIXED4FGL J0528.3+1817?ŽÿÛ$ÐÛÀ"zd×ñÀ;
mzVÞ3À<bً÷ðg@""¦ö¤b?ù£l-Î?ÒêsÜp®¿?Ó<'`
ª@Å@Ìxé÷@Ug"xû¿¿ïÿúŒ"¸'¿ïϯ l²?ïÿõMõVY?_³nØ¿ÇÔñžé9À¿é÷ƒŸ‡DWOTHERunk3FGL J0528.3+18151RXS J052829.6+181657?íBn ­Æ?´üY¨?qÜ®³±nµ?Š²/tß;?¶h! c"?´ã6»˜?éï$!ê­Ö?‰‹œ"We?prõŸ(?yò‹+Åf?Ç¿×ÏgåJ?ÂGwèÕ{?ë¸j­G÷;?¨ï‡{£©?'éœ÷R?e¿ą̈?¿ßvó|cÿ?§\‡£"?ìñ‰ó3hã?—Ÿ¶ª{³
?dÊúñ_î?UI˜y¦8?·Í_­Xj?—‹šÚ4µ?éI5sT`?¢Ÿ$¬Ì?wUºC ¥:?o;âü,?Ê |_ª"?*H[—?ãvcbꟵ?ʐY´§<?w¸rŸõR?ˆ~ŠÛ¡âú?Ø´Wo}	?Ê#°£S?çŠî^Ô?³8³:6?‹–BÀýˆB?†½qceB4?Ð
q+«a?²ö9xï?èeíi>KÚ?³G:°Úö?r½×x¹°~?r~Ŧ:ƒ?ÍÒ[ñ©6?³YŽY2AGN4FGL J0533.5+1449¿ß­¤%öÀ#•ÿ'+¾ËÀ:æí1Ç"iÀ<8|É:s@!M³ûo¢z?ø\'þ!?Ôèî Y'Â?Ùâwä"?þ ©¨ÛUý@_~ptZ¿çĀ}hák¿ìÃÏ,ù]O¿î—àÓ¿Û?èÙ¿y}¿æ©³ÊG¿ÐWÍÜÂ8IOTHERunk1RXS J053336.0+145115?í=¾"ÙI?°•Ë	dhñ?kkt¶\¬?l×ð8?µ;¦i‹´Õ?°T*©RÈp?ì	
ÙUyã?¹ÏßÀ‰6d?juñ''zÉ?i­òWÒû?¾ãù¨ç¯?¹Gߌ$ã?í3ƒK_¶?¤IH}2¶?…	V}֓¢?ƒ©Ì˜¥¢ï?³ÂºÖ#dh?£œÇ°à?îvs²x?'<:\¶þô?dƒFkõ	?`¿"þ§LJ?§P"žx¶?'+v6¤=?êŒwvüX"?¿pŠÊUN?{"²g¯[_?|…cw¸º?Äñ"ú¼þ?¿+%‡?怣ê^
Ö?Ë+/+š@;?wÄÇÓeX¤?ŽÂ\u:®k?ҟ¥薂?ʤ"ºë?ê;<ÜÕ-™?¯Ïê¢@tI?½äO?‡ÚXŒÅ1?ÄûP
ع?®©ŠgzÒ?ë ÞЬ?°$Düàñ?œïf4$e?†4Bé$??Àb¶ÈBhI?°J¤¨ôšAGN4FGL J0534.5+2201s¿æDùQ:/QÀ 6m
JÀ6"UõÕړÀ8{•É*€Ý@e
'àÃ@
Ÿ²$ªÚ4?Ð^beOæ?åLïg+ˆD?÷±ÇÞP'Ï@ î'š!¿ãq9"Ÿ"•¿í¦È •¡½¿ï·Á½ob¿ê tοêÑ¢ßé_*¿ï
²¢\·OTHERPWN3FGL J0534.5+2201sCrab Nebula?ÆU‡Š½"?Ê©…¡ê÷?aR–¨1Á?tâôÌY+3?êk;f;?ÊÐwSk|?ïˆo`h©?¤Z+Hêß?H‡l<¾Oû?pßÀíâñM?Œ[±ªç¶?£[}øOó¸?Ü$ÜG,ÿ?´4ª¿	Tb?À¤HÔÛ.?©dŒ"ï#?ۈÿOxZ§?µ>F¨)?ìŽWîËnj?µuq½¤¿&?'¯§ìÆ;?~ÔèT?»if·Ö?µt†Úе?ÁèQlqT?ǘÊJÖ+à?r¢Àõ¬&¨?­"íA–¶+?ë`¦<%†^?ÈxÔI9@?ð§?·Ý"1o®?|Ûié?Ú?¨Ëê1‰%]?£eˆQ?±êQ¸.…$?Ý-±üøö?´žR3P$á?¼¼ ôp™Š?¥/€¿m?Û£æà¨?µh†Ò"¬)?êPŒ¼*#?Æ ë‡˜Õ?=Ù=8¼ªV?A°"
ÉÚ?Æ®â÷0£Œ?Æ%"0›u´MIXED4FGL J0535.2-6736?їޒ‹ÍÀ@óGÀ9[‹]–´À;«qóbbÌ@<°®;Ž@ÅÊz5˜?µ	5'?ÈŸ‰ɺ@d:æ…Û?ý˜ä«㣿©òÕÊø6]¿ç$²1@ì¿æ¥Õ|ž·¿ëP™àç6¿ìC‡¿&›ö¿ï^²"&›uOTHERHMBLMC P3?ìTñå=º~?¬iÜ@÷Û³?±®Üo?¤âîÞdš?¨¥ƒöƒÐ;?cUÆÎ3"?å"EQä?ÇÛ(/I?ÎԞ:Æ®?Äurˆ]²
?¹z!]ú…b?«nrñ±€
?çÚãxµÉP?®§
~ ?¹¬}·eÝU?£¸}®ƒ?þ3Auì?§±9~"é2?ãÜ<ÉVm?¢d‰¬˜,?Ŷ½@(u? jnge‡?ÊØO=f#1?›[D Ã?æÃ;(–è?¿d͒£?ċM2…/Í?¶M¸£•³ë?ÀgÆ- t•?±ûç"Å_?Ù>	ºWÃû?É¥žñ®j?Ü?¯ƒCt?ÉúÖ;q¬Q?ÅË.o²ž?µ¯(\¢8?äjý1nŒû?²Ò6Áæa?ÃñPؾ%H?­ 'ßBñ?Êbºc­hG?«0‹0Ÿ¹?Ô5š­zç?¨€ºPx‡^?ÕS8f"?±×'×Ïùí?Ö­²µ…?¬ "c_GzMIXED4FGL J0537.8-6909¿ïõ!È°;$À?¾)Çy¦µÀ8ÿ[zz¢À;b8¦@!&±ú8•É@Dº"»äG?®!ý"L}~¿œÝÑ_Œ?òˆêõ¬À?þk,kÃÈl¿ïü,k˜ÕN?ïF2nè¿ÛU^–cY¿â/Ljp|¿åðª!§µ¿È÷gjW¿OTHERpwn0FGL J0538.4-6856N 157B?î"M©lö?¡1~#Ý°?d`Ś*òs?baóş?¬•b¸{? ™£Düi?îF‰=o»é?³¾ØŸ<;ˆ?•å^è'P?¦Ð@<û? ¤½A?ªNuÿ——?æ[ÓnÚ²?±'Yºp?—Zû®¸r?'f£þ|æ?ÑÒª$‰Õµ?±±Ÿ._ã?äuX@>?§ÒIV"¾?­i;‹yùÊ?¦úÿZ×?Óh(‰r@K?§J·¤?뎡…˜¨$?¶êøp?¾ëBÈ?uq/V?ÀÌÓøæX?µ_LIr÷?ì½—"u‡?À.iñqƒ?§6–vßO?¶«]oÕw'?³†È™–!?±õ¤a'¥?ã'By½?´§¿8û½?™{×{wP·?'ec;Dc?ؽ–N
¥?´˜ô`Ãô?Ùdb‡«ýÂ?®'iì¥&¸?¹Ò¾Õý?£8"ñœî?à‹$XF`?±»ÝŒÅMIXED4FGL J0540.3+2756e¿ØúLö‰¿÷ÿ@wÏDÀ7˜€dÀ:nÔw»ù@@ƒw3@$Ñ~uY?©f\^rT?¿úBPÝh&@•èO	R?þ`4:Å"ß¿ä7Ö ²Q¿Ò¯&ÿHJ¿ÞÐÏ%l¡¿âí±^\Vÿæ²Ô~«¿å¬Xž&ÇOTHERSNR3FGL J0540.3+2756eSim 147?š	VE%ð?"¸åQbz?ŠÔ}³C–?uô&l¡?îÇUü$Âò?ž'ɘpìÖ?ÇT'%%Q?Ä L?xh?ГûvÈ"?ĽÚí?áát¸þR›?ǘh0í?ÇE€)¦Ü?¯'-ÊÌ>?µTPÏ8R{?¢[±ÝQ¯?ç"à€ÍŠ?±•äùibð?Ä7+vŒŠy?«ñ\bÒ>?ºq*¶H78?¡YøF‡ª­?ç¤˓Ö{?´ó6·lÖR?˜÷ØRâ²?'
Gƒç±?–úʛvô?™Ý;	4iç?î€jèšøX?¢àL;¯èí?ªðS«ù»?©üÖÁ‰[?Ò5¸t·H<?ÈüŠ2Q¡?å6‹&?Ⱦ•ê¡?Ä<)ŸœÏ?«tÛ­Î ?²x—N¥Of?¢sëÉ·û?è¡é‹c9Ð?°âq›®Ï?´¤{ÙÙê[?¢~N¬T?½˜j¼Ù²?°%C­ëw?é¸c-nD¤?¸[fJe>OTHER4FGL J0608.6+1149¿íhtÛʸÀEà.©`·À:5.¬À;´¦Hԅ(@s¿®+L	@M»$-ܲ?Á™UQF¿›'ý\ÑV
?Ú³Z€)0%@eZwÅ´¿ßWú'ص8¿á˜f~9@é¿ê˜!"¥>¿×mÁðzÒ¿å'U¢ÉÄ¿ÛöUDz±™OTHERunkNVSS J060835+114942?î.ùiQÂ?¢['É•Ø?^­Œ*Rè?UÆ|uRˆ?¬ý	ë2?¢û?Êòâ?êßb›M\?¶ÒW'Ä?[¤ßWÇÇ¿?aîY½s,	?ÄK+Óԏ?¶¨ÆCñ?íC¦u¤Õ?Ÿ…•`ôÏ?Q¿n¢…?}²ÊËFa"?³¸"h¿í?õcÄËv‹?îs!M‹+Ë?a%ؓ=?]Rµ}O‰õ?A׬SÈÏ?§ãU}ʀù?Žw¥q ?ìØ'p =Q?«ÛñîDkÀ?t(N"C°R?là¿k¬s?·ü?•Oµ?««º¼E?ä˜îFïÿ?Å*ÌïÓ?jýGÆo?‹B͋)?֚
«™e?ÄÜ6_–=?êaã°û?°ƒ¯K?k?÷1J0íâ?‡ns6i¯­?ÅÃ\Ïþt?¯zÁQC?ëG1LµŸ?žOÐ¼?xn݊ŠŠ?d&4¢=ü?ÂÃâõ´?–­"ç÷øAGN4FGL J0608.8+2034c?ÉJ…ñWVå?֒*߈'À9Û©ßaûÀ:ɛëƒq9@™ðX˜—@"‡vf?Æ~ÿyó6?ÆûBÁp£+@0¦ždÚu@@®pì&¿ïÃvõ׈?ïÊÁ$"8¿èË[þ®qB¿åµ¦	êd¿ê°Ì†Uï÷¿ïÿÿ&¦³OTHERunk2FGL J0608.3+2037NVSS J060900+203746$?ÑrÎÿ'Ì?¿8â—âå?¹èÿÞG¡?°Ð¬ßªF¦?ä	xƒì«‡?ÁזTj»`?»øªqê9U?¹ë<ºËŒ?¼ìÉú+÷ø?²/*ì»ö(?èãQr}9Ö?¾Ar Cº?ÎØ@'µ?¯ö	iݪ›?Á gÁm?¥VgOKk?äêÂÅÑ ?±8)f1B?ОÐù_Ûe? z¿íHöÇ?Äj³
o:‡?œó[ºWp?â•ê¿ôC¬?£vj$íèT?Èjòt«"?·¦Fðz2?ÀgGñÊ÷Ï?³©·i8RØ?åËqeüfÌ?Ài;S¤S?¬%¿m˜Ô?©çý©ßC?Çò·øªKC?ÄÉ«R?è:¦1
B?ÅF}6{Uû?ÃöJ
"à?§‹U´¹è?àðé?ªy'¨g…?æ<'ÔböÎ?°6Tpõªt?º<C?"ˆ?–κ+Ã#í?Ê·ã³»{8?©;ÊQŸì?æ
vê©<á?©¹Ue{ô‡OTHER4FGL J0617.2+2234e?ë>éÆò\@DÚ`3FÀ5†õ)iÀ9ƒ~mÄ(¹@ —r،I@ýo¿«|?‹¼ê	Q@?À>¯þŠßí@6ú;šàÁ@$&žü?îxˆr)é¿ÐPF~êkÄ¿á_eÁ$øÞ¿áÅÞ,ñ{¿æ*Þ)£¿åWǂ
0ÛOTHERSNR3FGL J0617.2+2234eIC 443?±63p'º?°ƒç-Ȧ}?¼K™Ï}ó?Ä=ïšH?êOÌ_O×ë?Å欩¹Ý?ƒè¸
?žƒ‡çÃÞ?êçÑT4ÏY?Áœ^è:2ù?Ã":ƒoÇÊ?ÁN8Iiøº?ÆÝÅÃn)S?±ÀÕù•Yx?À¬¾ã2È]?©Oø½S?æ^ÖWÔ?µÞýHbä>ÿJ·Dá>ù'ûM?ìÎEÙå?©÷6ùSwþ?¿Ÿ™&ÆØ?©ö©ø¡?°×§x'ϕ?­~î×ëb/?»˜Ù¸ö?ÁOzš-›Í?êqïÙÂ(¯?ÃÔuã†ù?Œ<ˆ…¶?±ºsëê?êë`kz¢^?Ê]1Ç«Ù@?ʐåôo?ÈB"Ço7=?Áßõ,¬G?³àLö¶ê?¶þßï2`?¥·;Gâi?è¨>ح֒?¸'æù	>ÕÃ5‰˜>ÞYb%?ëb«€÷·1?µ]qñ?Âu&tÖ8(?µ]X(Ö¥ùMIXED4FGL J0618.1+7819¿ê¬4M(kž@8ݘ9GIkÀ;#''Œ6À<ÎYáÒ@Lû°>@D.ÛµÜ?ÀY3¢ï®¤¿µ;Šo°*?ð¦ªú-´?ô'ëí¤]Ã?ë8Åû!?¢‰grU¿å]Ðà؝f¿ÓÛ\Ý{›­¿ìÛ~WžÍ?Øý¥²¬OTHERsbg3FGL J0618.0+7819NGC 2146?ï4Wñ!?¢¸rÖò?~·ÇfQ?…~b2Yl?'ó1ÝÀ?šŸ§;z?îÊG*Xf?¢¢yIêp&?DˆÇG#?˜†y=‡	?—YÀë·?"ôٜ™T?î<Ž·ÏuÛ?›b—}<K?‰%•†|•Ú?†Å©ï‡tÄ?¥í¯ùàã?˜iúåœ?íðfèlf?ŒíDšu? b¹ºt¦2?ƒt—òô€? •O×àzt?ƒ2ÁŸýHÜ?îÀú¯ð.b?™Uƒð.£?Œç–U+%?‡neÇÆ?™lÞ܌
ú?"€§³¢T4?ìÕB¥t¡Æ?¸ÆR$"F?¢Î§,^–?¯œg	'ˆ°?¯Ý¸ÿÑ·?«T{ j€=?ís'ºk1?¡Æš®—'"?çùÈ2e?ŠÏnb•=Ã?°fëC'É? .m–Þ¹?éËk4¼?¨Åû¯Ÿ?»o97êÑ?¥4Ǚó`Ô?»škjvX?¢<f±Ï=AGN4FGL J0632.8+0550¿ÄÀ¬ÖÀÊ¿÷*°ãb:ˆÀ:b›!YÀ:ý³çùxý@!Ï¿4ïc@%!š"{$?À'¬î
46¿¸?³ÊnK@üR`õä@>bq`?í²µ)B©¿åèÍÿ|Í[¿í̌€V|Ž¿Ù÷›Â響à³Ü:þُ¿ß÷ë>Qõ@OTHERhmbHESS J0632+057?µh§¯?¶ç<§6v?l¶"e-?ûȵu.?í64uä™Ù?·~ZEh6m?Ò
ˆ…Ò?˧Q{{T?"O±Êç0?™+Þö³	´?æ^¾fØ|-?Êïçš?ÙÚÕG¶½?³×ï<NÀ?™Ö³{NF?¶#Ғër?âCßà0Ÿ?³.5jTŽv?Ñ`ª\+òD?²ïÎae?D3Çë?q·|p£]?ç'IÌ°P?³#AKð\?®È¾ö–?ªÁKj?z£¬ï—?uþ@.µ¥?íâ¼$€_X?¬B`¦¢°?Â¥s cé?ÀIÌãÚÇ?±åeI? 'yq³?êÑ8TI?Àlÿ<‹¡‰?Ï ­ù¼³¿?­ú"X#^?Ÿ 2bÕ?'(­V²?çw8F:?®V…=")w?²é×«Yì?£Å[úˆ¹ü?ˆ9×ŬЌ?"²ŒŒð?íAÝ¿}Ð?¥­D	OTHER4FGL J0634.2+0436e?ì†÷Xű¿û4ÂI¼´À7cx WÀ:]I.G;(@	G&…%@Ôó\ƒŽ•?§'/ÞêÝ?ͯº'ÈFÖ@"×\l¡?øá@âV¿Ô(þ;"»f¿Î…:¼êV ¿â†HÿxE·¿ç"O…yQ¿åYÏ^ø]õ¿èxŸN€ÌOTHERsnr3FGL J0634.1+0424Rosette?"ÀR:É©?"êØ t?Ë¥ú^¾?ÇY=57Û?èx·1ŸC?ÇÄmÍãÎ?ÖE00«a?¯tfŸÀQ?æüùe啤?Áu[<ÍÌã?Ð(¨àßSb?¿•o…Z.?¼
bHc_æ?¦Q$ž'm?Ö½Zy7?µWÏ÷Xú^?á (‰¶øz?¶1ÅåÞÞÌ?'¯|b"¸?xuM±Ò0?Û=Fÿ».?µJçë…Kc?áËàRûi?µ"žBuÆV?‰+iäjæ7?'{E ;¤?дãiàz?Ħ*Áʐ2?ç@à¤a
?Äâ_Ə?ŠÑid~¢?¤ÁWŒyš?è¼L­¾ÐÇ?Â˾ñô
?Ë6 1'û?Á™k°lÕ?µRÅ?¢åDUÙ÷?֗>/»"{?¶\°\¹g?âv©UÏ?¸ìkÄ6`?wÆâåÙ\T?e6æ[4g?ÛS¸¤KÏ6?½ôoNӈå?â&•è#T?¾'¿Œ\ÈMIXED4FGL J0639.4+0655e¿×bN
?àŸS À7 /^'\ŽÀ9À¡²lÏ6@o½fþ;Û@a&Á4é?´b_£ÿ?ÏÆæxFä@X_^4h½@@í°òý?ïÚ䜸2¿× (ú¿åcÀEç¿äŠ]âsA¿ëÉF/9Ä¿æJe~ßÙðOTHERSNR3FGL J0640.9+0752Monoceros?'äÚÉÞZ'?"âø®-Ï?ÇaP}	Û?Å#M'>ß?éÜ&Å¢·?Ņ!€a?«,$N©?¹Ô§ö-?ãq¡
¯º?Ç8)±æS?փšyhv·?Å-ÌòÙ¯?¿ÁÖ0›Î?©RqÚìRØ?ÕÒÖÃE?³c]ouBr?áYØlä?´¶oçd?Õ?•¦á¯²?ˆA¨Sâ#x?À§²$ï'c?²Ü‹Oì¢?ë)&?g:?µšJ¦ÑÂS?s×Öð*°?j
?îRß?Í@¼€?†kÌND(?蒌´Ê?¢¾•kPu?"3¤mF?£ÌÉ
Mç?ã·Øh"ò?ËofÊåA
?×^¨"›z?ʂ9mVg?¸†B)|Bt?¥Ò²¿ÛLÂ?׀À§'?·ÛõØ|?á.×gk°8?¸¨…ŒÉî?ƒ
åpaƒÕ?xƒ*ÖÉ?ÃTϟ(ér?»Q¼œd5p?êÞ 'I¤l?¼¢d	ʯMIXED4FGL J0647.7+0031¿snŒ"™¿âN»ßê‹ÐÀ9p°;œŽAÀ;X4Ò@ŸÕŒcûþ@ÀùÅS[È?⡟øXkÒ?ÃÆe¿øS
?ÿ€–"TÜ@‡f$w-´?ïÿhJí¿º¯÷¤ç«¿éºÄöJ¿êÒêRï'¿ä

ù½Ç¿áÓàx"OTHERspp3FGL J0647.6+0032SNR G213.0-00.6?êâG7C…ˆ?´=§"?u"Á×¹'?s7öŽ¬žŒ?ÃήüN¼ô?³½)ùÞÕ?ãfdÒ¬O?Êéâù?Ží"
§n«?Ô—5UB?ØÕÇíkí?É·dþ?çe!Òü?¬àhÚ
Ø3?¥Çÿl3]?•÷­? £Ð?Ìù³ +9?ªr2XŠ?ê!BšÚ6m?œÔ§¹LOT?'ŒÛeÙÞ	?¸ÍŽ®!?Å)Z'¤ðÌ?œ ´ÁÒÄ?âÅ¥ï·?ÒfiÁdº?"B©·?ˆ$H¬
±ç?ÙÒ ~î¦?ÃvœÙ-òñ?Ó½Šçœ~H?Èþ¼¸FqÃ?"LŠ±/Ã?š)"È?å~Ö7=ž?Ȉ4Ï7Á?Ýq™¦ì?²Ó¥ZÍ=ü?µs(*ó?¡ÿmýÂ4¯?Ý29eHÑw?³' BM?ã†;1É ?¸"h_-ð¦?–»6+O@?œ¯x)(?ׇÖ:V4Œ?·lïƒMU]MIXED4FGL J0650.6+2055?çø×:ËJ@"h/"BAÄÀ9æۚÅé"À< öðŒÅ@ úe	.O?û

jKÎ5?¼a%r†Û?³d' +C¦?ûVʗhfò@VX§6?ïðHgwÞ^¿æ¨
/"k'¿Ó6@®ÆÒ¿Öµ@S­&>¿ÖasÕB<¿Þ·a`m("OTHERunk3FGL J0650.5+2055NVSS J065035+205556?îf@fL&?®o¯Ž™"‹?aÉQ 
;ã?Qþ¥ëÂ?¨d€†mÛ?®g/oFnU?ê2CŠªy¢?Á9@Š×z?uf·ÚK_U?zê$Wía¡?Ƌ¼J^?ÀÞC?£a¢?î+¼Ã"Ž?"kSÌ`	c?tS¨½?hyxÓ*¨Ù?ª²ß±€ì?"ä—7ÍH^?í«îäW`˜?ƒœÝ$?›¾?‹.}&?\ÆÒéB¸…?°|×vÉàß?ƒDà·í?ëÀmô$Tž?³‰AGÃÅ?}‹èBo?nœ%7	"?ÀèíŒ,k?³Cpæ± -?ãacн{?É%#xޖ¬?"r3Ñ66?]9ë)?ÙO«™¡QI?Èá¥üÔQ?ë^˜=gÙG?§Ø`ýçd?ƒ¹b°y?uég,÷ê9?ÁSÃtg
´?¦‰G֝ù?êP/§pG?š•^$I›?'×Á%Æ?xú®N'?ĄIgõT"?™Èá׎AGN4FGL J0709.7-3009¿ïë½>ÿ"À#J½ÂmÎ:À:—¥ßøù|À<b+¡ƒs@ Šý?ÿGKƒŒ?ÁY:?w9gïlMË?¹Q8½òÐ~@F¸4Õ?ïÿК·¦Ë¿éiüp¿Ô/(âwXý¿ãŽþ "of¿ÕŸ{¿ßއŸÇ8OTHERunk1RXS J070947.9-300901?ì÷é‹tgÜ?¶$Æ0Ùð)?`)M\yZŽ?XtRàg&\?·¿i7×%Ï?¶	*nÓK?ì+'ø¡?¸êÒO6­?\>‡=¹+€?ds¥k'©?¾3	WA°O?¸µ+'é£?íÿ'¢‡ª?›Ç¥y)j?hö­íøº;?g6×ÿ·?®wƒ'
÷??š¿Þ*Væx?ï?Ã\êl?t2S9o¨?SSS4›?6ôMèE¢?–Ò_-ÃúÅ?t4‡n»Hè?迓EÚD?ÆGy³—"?o¤Å ¢ä#?cÂyµï'Ð?̃ n¾a?ÃrƒU4Õ?ç<ª*`{Á?ÆoÔ#XJ?^‰Vï‡@?oÈݬ©xØ?Ñh"UaÓ§?Æ
Ò ¡?ëJ¨["?§ 6x¯`£?wkšc*^?rY˜K¤ê?¦:"?¦ï¡=Eék?í°CÃ_vï?'TIêjþ?i½æú6M?X+֓ç%X?±¯ò¶SÒ?'f3WôFAGN4FGL J0744.0-2525¿ëJ¯×|0Ü¿ç§ÃÉfÀ8Ï}ÓjuÀÀ;z鳍a@Š9-s*Å@¡½aõ¾^?³ÝLvѵ?Úͳ\cX?@#HÈ/ù?ÿŸlÊX©9?äJSá)¿ÓI }8é¿ÜY"åO¥…¿åßÖÊ|t¿ð?ïÿÑqw;¡OTHERbin3FGL J0744.1-25231FGL J0744.1-2523?\çÿ€˂?c`Ǿäy?î|sVõì<?¬f9GƒÔ	?§QŠ˜<$Þ?«ÛS(j.&?mÏÍnn"?¤ÚqfyЉ?æëRô;/?ÁÓïsôL ?ÐR}²Þº?Á	•H.Ëx? úq˜ñƒ?–ëì, ŠÞ?ëEeËòî?«'ŸÖ?Tc?¾ðœ•ÒK?¨6#›™+¾?°z"têÕ?"o×^c?ãè=~ï&ò?²8 µÔÿ?Ôãå9¢…?°ÚÝU?€Ùàc†ýÖ?°Oà\ˆŒ?î=ÂYB£?¶${—G|8?§ífé^?®ˆo CN?ŽªßCQ¨?¡ªÓ¬®Ž?çBíÊb(-?ÇêW œñ?ЄÍqYÖØ?Ç
Ÿ"
O?"€zz†?ŠE"áª4?ë¦^ìt‡ç?«uÁÚõ?½ìê½9e?©b]&Ó|µ?ŽÂŽ…i`í?yð2ÏØgW?ä¶á±"éà?¸†¢¡?՜((¬á9?·¢Þ·#ûÚPSR4FGL J0809.5-4714?ØéՉðëÀd]wª\À:
%ÍïâÀ;ÏVØSéŒ@Á…§IZ'@*N뒋?Ã'CeÛQ?ºH"Cnj?õS½vd?ýŖ­V¿ÙT:귙¿×ä[Ê+1Ý¿çý'1ÆK©¿åÈØ\œ8¿ãف±E‡Ê¿ïÿîÝÃÀ	OTHERunkGamma02 Velorum?ëíãà刅?¯I'T('G?y&÷šÂd?h3þÑT
Œ?¾þqïÑ+?®Ê'¨òB¡?ét7p•Ð?¼'ê¾O[ˆ?y"FòêÛ?w7vn?Êêê…U¦?¼?¶íEð?ìŸ<¸ºh"?Ÿ> í*ù?'J~G¤?"ªF¡5U‰?¶³"ø5û?œ ëXº?ì1ãÿæ¢?Œ:ž
$?'hÜ7xè?mÊ¥fg¤:?¹Ö¨òìµå?‰ãëÕÚF?çѪl¥š¯?º©ÎIhm–?†ÉÿB3äÛ?vcÏ£
ð?ÏL¶Z"=ö?º|ÏÜÌ
?áCPTß³ã?ȁäsT?ŠFˆî¦'?'¶t¬á[?ܧ.Áù#?ÈH‡Ù~?è¡G2×?«iº¼{‡:?£IÛeGÖ¤?'4ºßÉÛ?Êû
Ú,9?©âi Ud?æßP%Ão<?¡ÁÇ"¨Ä?¦Þ~Dy?‰"TŸ±º?Îý΀×s? lŦ÷úAGN4FGL J0816.0-2342?ÍNâÏv(@o4þåMÍÀ:SŠ ÒHÀ;Þ€@J‹¿f\Ö@–Ÿ¸g?ШÄûb?Ó.ƒ€Óz@¡zSƒ5@ˆ`â¿ßRBã)…Š¿ç±/Lô¥Y¿èђ>†x€¿ï[nÎ?¿ïu'>³D¿ïªáö)½iOTHERunkAT20G J081524-233846?íZj8",?ªzRÔÔ§8?…zÁ£_&g?|‡)xøûÜ?²€tz=mP?¨Ñ»H:ãH?媣"*€?ÃSÜ1Tó?­Tgîù3?¦Ô†™PP?Ðü
+kØZ?Á}\¢lƒ?éÊ®
ّ›?¨›è¤<â?«V"
øíæ?™°2|íK?Áÿ¢ÑÀkY?£ËI»œ	?é¬M?› x/6…j?­Öb#•ï1?‹þ~°&ß?ÁÙ33Da??–4©f&‹Á?ê"˜&c?»•™N?˜gn«ÁŽ?}Kï½s±?Äå4'?ºN~,¨?×ç[<_?Èãta¯P?ÁHþ´Ùï~?»#°ð^ˆˆ?ßthK‡¬¡?Èͪãmù?ä0ÛýÂ8?±I à'ü?»Œ\•éG?¤¼¶îsy?л0ß=ÿ?¬•Ì‹±?áxjÖS'?­9³mÓ?¿Öš9c?¤ª;Èñ–?Õ+4ÑîÊ£?¬:q}@*MIXED4FGL J0819.5-3439¿Õ9–Т«w?ëû=#JÀ9ÕÊÛ[	À;zºÖ*D@ég)ÚÄÝ@":ÚÇa?ÎTð]-Ù?Ø"Ÿ€&@þ'Z·Ü{@¼L0Z;?ëˆÒ!Š_¿Õ(,ÚSž
¿êÒiY_í¦¿èÓÀ§$œ—¿ïþP¤]B¿¤­ÝTOTHERunkNVSS J081945-344215?ãåÒ©ýâ;?ÀtèÄ=öÊ?—ÅèNâ0?ŠaY	§5É?Ö·ü&'Í?À8YpK[?äÛ<™/Þ·?Ðòóty?¨ø`u÷Ù?¥Úï"»?ÓIGÁ#?Í£è'Lã?äÑÚØu™×?±€F™8î?®Çuød1+?™ó9mëÞ
?҃[Z¼Ë?°;…Q¹E?䖗ÈÓ³?¤
ýÁÙ¡?¹òR?"Ó(z?Џ/і?£$kqÍ~¢?Ö8x
Âj?ÀçT.ø³?¥¥
/ÝK?›àküWÙ?ã‰s'®´x?ÀÂ!N½l?Óh,(x?Ð@—U?¼Gƒz"ø?½ÍÞü?âÂùœ0E?Ѕäaz)£?ØXvÔr³|?´\zògû?¹ì>píª?¢Júq˜?à–<Ǩíí?µ`-ÑWG¦?ÕjÍqkä?¨­\Né?Ç6ß5ì1R?£u$*'â?ÞùÂóžâs?­ôxº\ÒMIXED4FGL J0822.1-4253e¿ìè»Z+À
þ€{»bAÀ7M—üágÀ:ª}ÞR0N@ƒexy?þ"Á-\Y?Ñ÷À&²X?¹Í½7®m@Ìx £
·@XðCõMJ¿Åi€Íú¿Ògáæl¿Þ=êg9 ¿Ü­¤"r¹¿äŠS«x¿.¿âgk*NOTHERSNR3FGL J0822.6-4250ePuppis A?Ój¾àP]?›­6N?Æû˜¥†jp?Âà-e–<?à‹ºfv_5?įà¿FÃ?Ç	…©'x?Æ2E¢vŒú?×c»AÆ/5?Ë*èþã?Ý?ûe?ÈÓõ'xI#?Ô­÷LÛ®p?³¾;?;í?ÀâBu‰C?¨÷÷Cª
?áps¼Ôö×?µ¹^D©´6?Æ
YÀe¶=?¢5‡~|?Ê|¹'?§Þ/EžâÝ?ã÷h1AÁk?±Lø¨F%k?ѕØö7?ÀrÜ%§§?²ì³^5V?­5|®dGv?ä×}$v7?Á
1R·Ã?³Á#Áé(?¼ÂÐÎÓÑé?ܲ¾XÀ¶?Ð_'¸¡>?ß#œù[²??ÎT4[bz?ÐÍx@X‹?²l¢'£+??¼©7ö€>C?§o˸!Zs?äIEËò?µ=V©HÎ?³ÿ8o]0?˜)·\ýi?ÍdÍ`º'?³4Ö¦‰?æ&å«|+[?µÔ–ŽwÙOTHER4FGL J0833.1-4511e?ëa…DçªÀÙ0¾
í)À6¿Þ^sSÀ9BY`Äeö@!ägÀ`@QŠ¡¯Ñ?¦¤©;?¡ÙÖ~/
'?ô,Áÿê1@ãhšž&q?æU€e.?ҩ… ¿à8¸¾M<¿Þ¾u5¬¿ç=ñ7¿âµÚPp[OTHERPWN3FGL J0833.1-4511eVela X?z½.' 
?uùŠ±þw
?R"ò}F`ç?`¤à~î8&?ïÁt)¦B?y2K'»€Ò?Ót'=²h?ϙ'/ùš?ºÚ¤ïÁ¡ÿ?À¿Ó>ÖÕ?âêjC.—²?Í–k^?H?¸5`•r?¥"ùË¥³Ã?ª	jVéy? Õlk~¢I?ëX½ír
?«ØC_Ò?¢AԔJ?‹RD¦Ct?«a©…xd?•íÇi·*?í)ÔC}r
?œÕçصÆó?ˆâéu£:ð?ƒL¤Hç?uÌv"b†?®Cœ}f?ïpÛlͳ¨?®UŽw֜?ÇÎÊ2¾™-?É[íܼÙæ?À>óى§<?Åvy±U??åü|íïæ?̽Î}ãö?»~ÝYüw?§Æ°¥"?¦ŸÄT8?%E]" ?ë0Xµ'?­2l>æœa?£éIrIO?€Öâ¾¾Nª?²;r&¸ü`?£ì,ò#ô?í3rqGé?¥[Ç'¿/OTHER4FGL J0838.7-2827?çMàØ8ç@=5¤&»À9"©¥€W©À<pÛs@Í(+˜4??þv9ïå×?³€šëSK?Ó3\£Äì@ïbùÊ\@$ïªGfÇ?ïõT9¿¯ÏÛ Ñ¿Ü{ÔA‹:±¿ÞœÆtÃ÷;¿í­òˆH8¿ïâ."'AÜOTHERbin3FGL J0838.8-2829XMMU J083850.3-282756?§///§ê>?¥ÙrÊ¥?쬩)79†?¶O-×jÛ?®>A0a?ªó2r[ ¿?±¯Y-ô?¶KØrQ¿?æÆb­ý²P?Ä,¼ðWA?ÌÈ°2F?Áía³èê?¼69s¥Ol?§ÿ"™¨L?é°â¸?±KG¯"4?»4EíJÖ?¤–újÛ9N?Ó`eStyØ?§=u÷¬?àûî̸8?ª<'Àv?ÅOz&6Ën?šGO;?‰&GêÒ?'ˆCê?î*" È? H¥K
 ?§jAK֖?šû¿-ÆÅs? µRþB?¦"µ÷C$?èL€¼e?ÆÇœDCÒ?ÊËü_Ü?ÅEh€âq?£b¶'F?™JKÅԟ¥?ìÀÄMCÍ?§'ªz"Â?µ¸žÓ8xw?¢0¡g×R?Á)¸9í·? €Š"n¡?äÑC¤=?±
1ZùQ?ˑc·ÙV?¨‡Ov'' PSR4FGL J0851.9-4620e¿æÚÉHº{¿ó·þ½à¡À6Õ6$;JÀ:p³"&k@!²KH¨»K?üßѧ' Ö?'Jf¢î¤Z¿"¿g€å?ûÄ¿9aK@:=,0_™?ï	H]ç¼½¿Ö©CEO¿âm)c¦˜†¿Ûd`½/þ¿Û±€@,?ú¿È ƒxÅäOTHERSNR3FGL J0852.7-4631eRX J0852.0-4622?ÂhƒŒ'ô4?¹°
šôɧ?Žz…ŠÌÓ?•e'?êëõ°Pô?»e¹ä"?ÖO'|ƒx?Äp!Ñï?¬ÈœÃCô?¯Ã<ùW/Â?éMâOQ23?Åh™‹E²«?Ì}Çô6¸?¯NÝëz"M?£eÍ¡Ikx?›	l‡µ
?çª1_|
?°¶""_œ
?Ôõ¹[˜?²!@šäm3?¶'Û²÷AH?°-›ò?â³A­8K»?²³}ò'Zð?¹¸m3#Ú?±Øï^Hêè?‡!¶×Þ?"OP2¢Ë?ìlk5þ?³!Áéqµ?½5)Øk't?ÀRú"ñFª?¦¿c5Ð	?±Ú¤€"H?êíbΣ³ñ?ÂT¨dÛ?ÁØês¯?¬ÛCŠ¨ÁÔ?–·a«–œ9?S`‰´r"?êÔ@qè®2?­š¨—¡7l?Åé<ˆ?°³'2/¸?¾G~³~
?®"<î¦o?æ¼Á#Ì7ü?µrŸEFŒOTHER4FGL J0852.5-3123¿îƒ$Bˆp@ ½óùa€NÀ;,%5À<ƒ·'¸¬"@">NÃ9%?ö.­ýÔ¬•?ÑàÙ^«‡?ÏÈžžç?ôŠB®Ñ9C@2õ#Øø)?ïf¿2Zp¿ïÿQ^ÂX*?ïüÉÚ¨X¿Ùoß¡eÀÏ¿Èø»h {¿Ð$—Žý^OTHERunkNVSS J085238-312331?î0¥×7j?¦éö£;Ø?[ÑO³²wŸ?OãEø¿?¬È%?¦¬¢‹µÊ5?çŽaˋ??ÄAþÏD?ƒ#n²Ò|?Œ²QyÙۊ?ÐJ"j…|N?ëqƟiÆ?ìÑE–Ñ×è? êsù7i?u
ñê‹?rbû¦=¼°?¸%$? šr¥—‡N?íq±'w4·?'t繋r?Wù2ò?IܼrÑG ?´'ý€å<?']˜Å/àÈ?ëøÏÍø?¸Z‰µâ)Ê?k|$SÊj
?^Õt»d¬¿?Ãb,÷@$?¸5Ï´åx¶?à)~86Ÿœ?ÉI¹&Ò§­?‹2£‹ø֝?—§y7@·j?ÞÓnsód3?ȃ>ªEõi?é)ž¡l2?­k<ÖHlC?€á%›ÜD-?wK'É¢"?ÊKu&ü Ö?­ax;·!{?éx{ƒÑR»?®U<É98i?bxae?a·.‹žÑ1?ÉÔ/µ­Ôî?®H©rdòAGN4FGL J0858.0-3130¿Ûß÷ªy™@"dj ‡ÊdÀ:^Y­ñ?sÀ<6×%ì"Ó@!±Ÿˆñ֝?úÍwҟt¥?ÃñîšQûJ?·ø™Àl''?öf2ƒ
@!Uå?ïâO`:}T¿ìénù²Þå?'îSžýJˆ¿Ñ«ýI2¿Ôž[JS‹¿ØUd.(OTHERunk3FGL J0858.1-3130NVSS J085802-313040?í9ø6‡üc?¯}ªlþð†?X8z·­‰?G¸2ùUð?µÏ\`ËiB?¯].ð'?éÒgäÉKl?ÂçºÏISÜ?t,tybæ)?zw-±DÐ?ÈüÉ66À?£èŸ] <?íiKU
jß?¡äÓLðR÷?iÔ6¥çÜL?\¬öÊŽ?³ç¢gl¢?¡ÑjnÈZƒ?îRÍïC?t
B+?cuÛ³tS?FhkK†_E?©›ÐiZ#Ç?wvð
¸?è£;†"Øe?ÁWBM¾…?gÍêBÏ>‰?X岜«äù?ÍÚ<÷Ø?ÁO1&ϳÃ?ãKhf?Çd,‹X¨?z-¾©kÐ?†¿%SÓe
?ÙxÎüZ?Çù³'n?é&ç'ö½6?³ŠI~ª^?v'a¬P?n2B'¿;?ʯÝ*	‹;?³Vu3‡»?ë9Ø´•& ?šñº-I ?vMPÂDŽž?eRö^Îçä?Âf2¨¸Š9?šîNÈR#?AGN4FGL J0904.7-4908c?íŽÊí	êK¿öú@óæJÀ8ÖÞZ"ÊÀ:Z¿»lR9@\´5ý@	STÛúg:?Ð@rM'À?ß݊àY@ŸÖjÛ@@j>NX(¿ìîàwW?ÛO®~ƒÄ¿ëU£ ƒ˜¦¿êÐäôá¾Ì¿êž–Xœy¿ïÿG]â‰MOTHERunk3FGL J0905.6-49171RXS J090505.3-4903244?°Ÿ)"†¶ç?°©‡,ÂqM?'Š§È¸>k?"‹h,÷ö?í_ŏŽ_?²ru‰?Ë:h0Àè?Ã'V"F ?ÉxNµ¤®?ÁOÀ²0€?âÚ]¸(6;?ÿîñJt?ÉG³þ?¯ÐÒl©3†?¾ÆS݈íá?¥›^
_‹?åÕQVÅð¡?²{
Q3Z?µO"¤ÓŽ§?"–u…·É?Ò¹A¸±—?­.–øFÒ?ãùl92@?¬mß´3q?˜;¡ÈrÁ?œldåÚPH?–Öç,«w?š¥QCû"?î‡r"Õ~?¦1ä4º 9?±ì}@)?¹ÿ¼#·^?Ó£–C_?˧-Ø]?ãð¥:rÓÃ?ËCÙµ¶—?ûÉQ9¥à?­¬@@ˆê?¿Ì›9+ðŸ?¦ÿº=†¦Ö?çzDŒt?³(Αò&?"eã^´–?}²TÏØê?ؗê<ŸB¦?¶Œ5‹ó«Ã?ão²Ú!8?¶J¹î•øºOTHER4FGL J0910.0+4257¿åpîÈ}»@EvFbºà;À:i—Sn<À<{8bG@è!©s~@<¡pþp?ÎêÒñ±‰?ÓЧ¸@MÎ@5@%Nn@·'ŒYë?íݻŽZv¿äðÄ"ð¿äÅõãF‹Ö¿ìÒÏæ\ÀË¿ïì¿EûŒÔ?ï¦ë\ÕOTHERcss3C 216?ï$æÌÇ?Ÿ%ûî÷±?q|B7h?n÷ŠJz,V?—2¸0ò?œ7ˆòT´?î6w‹QØ?²åۈÁ,?œç‹/?¯Ë"Éä÷!?ŸÑ¥ýê¡Ö?˜-kYá?îs«s`ÊÆ?—Þ€‰?Ù	¦Yáí?‰,þ 5hb?¡O^¥
&?'õ:"gh?î Z•Â
?" (óÌèg?•¿`õۆ?y³Í-äút?–Ûýg*xÓ?x9·Ç#?í¸>Yú>Â?©>Jôˆ/?…èïX˜?ë"â?¯ކÆs»?§Žb 4¥?ë'¾OÜa??¾pOUJ+À?±‡ý½j
3?µø0o1Ü´?µ:ÂiT?ª#˵kI_?ì«ü¬¨-ö?¢«(äÚór? áì"þ ?"‹¡Èâéa?²/$Wc™K?šÉ.1Á™?ëƪi©?£J¨ÐÜ5|?«ZaÊp24?šRòå<·?´{ËÇL?˜¯¯r®O2AGN4FGL J0912.1-6449?êò\QBE}À&n8§ç:6À:œJNìÀ<=²ôݍ@u±ô¯>ò@‡È
±™?ãHv;?Ê#ðõöç¨@æ;ƒcÍ/@)åËv`"?ï^·E|¿ÃjÓÞcøù¿ãíŸ
⵿ä`³Ô®Bž¿ìª0À',¿ïè,9CîlOTHERglc3FGL J0912.2-6452NGC 2808?ë¹#i*Ê?°Þ"{µk?™nµõ߄?‹¦¼pGáw?»Ûb‰.‰Î?®Ù Þ4
?êŽ~ceފ?ÀúÂ.õG&?›Å£¿J? M)h)??ÂMR¹¨Ð?¾|+¬xØ?íidY_±…?žò•#â4?Þ~óG'B?"-:%ÛÃ?ªzzìñŠ?"sev~í?í
\¬Ëœî?…3¯‹ã-?¦¹ÕÊŠL?|ªVGÇÏ?¨ _f¯ñÒ?|{?':u?æjìš>ýc?¿`¾Y!Ú?®q$ø‹V0?£òx/¡	N?θW—Zi?¼M~IBOl?çìÇF®™?Èܝ…˜?®FнÕàˆ?°>4?ÌZ˜´¹§ù?Ç&ÆÖ?éDºê¢Ð?°É²|n¯n?µ*Ì>ÁãŽ?¤½ƒÈeΫ?ÀW®6Mˆ¹?¥ûc©–¾}?égÿÿ1×q?›rú,¶?¸$}l¸,?•Æeù…Ǿ?¼›'›É?'í\f¿·AGN4FGL J0921.7-6317?áø䞶ËÀ"Í$žDúÀ:÷I,™»þÀ<¨p˜ïO¯@µÃvâµl@oÿ^ðP`?ÍbvAЯÛ?àÆýòÿf@}ñ'Ž»?ïþޔY#¿ïýSõËÊ?ïÿ¢­>'¿Ø†±_ˆü"¿áÔêp6Ê¿ïÿâÙ~‹÷¿¹à—/'âOTHERlmb2S 0921-630?áqp0о…?Î=‰©È¢?ÕêJ+rIŸ?ʀ:Ôè$?¼ËUÇebc?ÂJM½3?ΝÌåD?Ç–*?ׯh˜šÁ?ÅúžÒq/?Ù±arœç?ÈLI¸8sÂ?በuœ?´$¬E'Ü?Ò I·6ì?³4n)zãü?ĘìD%7·?§âǜ'í?ßeº¢†ZÖ?¨pÇm†N?ØÈ^|üĦ?©Q«–î?¿G›ó'?—Hi€k-?Õèð"%Œ?Ç(j enL?à˜.:ƒ'$?Éâ0ÑÊÊ?ÁÏ%4ËlX?¸ÓA!ô¡œ?½9!ùhÑ?Á®•}?ß?³²}ì?ÍhZ©¼õ?Ù|>‡à?ÍZ0"Š{?ًÆÈ%ô?µxÃèaN?ـ‰"ÅïZ?¹FÑ°î<7?Éç_f(9@?¯4]Á"Ã?Ð0=Ùï?¨C'Îd¬œ?᜕ý$Oã?²Ô¬Ž?É-,W¤l?§³tV×ÇMIXED4FGL J0935.3+0901?¸&S%ìΠ@D1'€w‰¤À:&<ì™.À<‰w¦×@	ÌžT@êû܄е?Åˆ¤~Ïê?Ӌ'Û9w@
¸«ôÌ@Ûa:,¢¿èÌ~=šZ¿Ð§ýàk¿ãèÖt¿ëp×£Àd	¿é g´D?Ë¿ïü²ÙÀ3OTHERbin3FGL J0935.2+09034FGL J0935.3+0901?튽!¢×?«tdxGð?¢ë$}m&?›±/H©"_?¬œ/¯œÅ†?¢¶™­d©?ï@ŸðuÉ[?Ô'ècž?¾%mƹ?'/ÅÜíÓ?øñ`-{ß?"Êv—1?ì7SNÇj?¥u̬]Äì?«aÏýԍ©?œR–d€¿?°"}ç}Ú?›ºH‰ÞE?íìµ:èfå?‰.糨Åy?"?;6Õ?rVìEÄø?§•!3Þ'3?… 	Ž2Øü?çÑ¥0‰"?¼¾n˜Â?¶ÙDuýÊ?®À²¿
?ÅLÉHí?´!ÛDèE?턓èՖö?²RåÄo¥?ÓöÿÔ §?§ºA^2ÿö?¨ÌÅó˜'O?£ahz½¶Y?ç'V±èp?³Ñ¯ã—?Á=¾ýVW{?«÷_è/ð,?ÀÄ7§âÆ?¦Q$8X0û?ëe
'8mÉ?¡¦^…
É×?¡úêÿS6þ?‹4ß} «?»Úoéµ?Ÿíñ
2"\AGN4FGL J0951.7-5328¿ª{ø.[zS?àœ2#iÀ:,F)¯ü²À;€U&£ø@ *úõÿöñ@Ï=ÀTïF?»•«ß}´¿·tA4A•?ùÑ(çÖz@o…'Ñ~b¿ïÿKâCW?ïø›AåR«¿èí][zпÜÅåNë ¿æ—â?$Øý¿ßFôçôOTHERsppSNR G279.0+01.1?äÂÎw­ò¨?ÅSOãÿ*?tGør.$?o©­ìÂv?Ö)C.¤ï?ÅS·«R?ېƒh³P?ÐMzÙÝMñ?†kUß;¬'?&ýAu?áÞI旽æ?Ïóó-N?å¨6äSã=?±G™œEð?˜Äܹ5¢?×¨+—?Ó#Dkrrl?°ŸCçžOÛ?éà£q'G?Ÿdê'F??Äâ²7+X?qì
Iù?Æ¡$ÝKS?–t쩝?Þµ–WùD?Ŧð9Žl?':\'ë2?ŽÎäoÅÇ?àhROê4M?ÅÚa4ù1?ӖeþÈ®–?É^?£S?"ÚÆé­Ö?§5'x@¸À?å•öɗÛv?ÈÂö2){'?ÞsÖÁÝ?³¶Êeû0?§o$d´¹?˜)@d§?Þø¨eíÎ-?²ÏYë"õ+?âùŠµÑÅ?²J+to`? T‡£šEÞ?‹/W×8}Î?ØYŸa7[?±Ø;"²'|MIXED4FGL J0955.3-3949?ïGäΩÏ@'ì9yžRÀ93"P>ÝÀ;¦d—YMy@³›­E@óþ?¶=̀{æU?Ñ¥«`@‡…@ñ'©"á@THV±?íêhô¶â¿ÜÞdå1óm¿ä†2Ÿ£‡¿æÆŠÁX¿î¬­½½æ*¿ïÙî§z-OTHERbin2FGL J0955.0-3949CRTS J095527.8-394752?ÑúPë¢G`?Å`›m¦˜þ?ä"ÿÓ¬²H?ÈÀÐ¾}?³î½´í7D?ª.!
‡K:?ÇFÁOÁs?ÄÎlƒ¥«:?æc§ŽiK?Çn6`܆ ?¾U@Ü
¤Á?»;g|"6?ވQ‡œ}?´lƒ¡_¶Ÿ?Ø=F³~Ù5?³•Gè[zx?ÂtÐeÍS?¨ €Œ¯Î?Ûwµiêæz?¦-eUÿ—Ï?֒¿ÄÀR°?¥@¾½é¥¹?Ëë¤ÏO+?›u¹{È^?³î¡¥˜¸?ª_I3?ê¨^?¹r3'.?»éE˜)pÖ?±·h*+µ?²Æ¦"°ö¥?¶ˆ¢?êÖy¤]?Â%zvF`ë?¼Ú¥¬¼$ù?ºê cI?Îç
¤È½?²8
Hpkª?âÎí8Ÿ{?¶_÷™ž?Åà†¦UrV?¬ûåÉZíÛ?ÈCA7¹ß? ó¯Rÿ(?à43"¢ø¤?®H?Óuø[,1È?¨x›ÕۀMIXED4FGL J0955.7+6940¿ïò²,LÃ@DH¼ƒ©mLÀ9EMÐÀ<_¶Q`Dä@‡•;;~@[­}|,¡?¨Ù#ƒy?®ø¤
]X@ç*ÙÈ]Ò?ü֘UKáÖ?ïÿ ~æ¿à+RÿTÿ¿á¶Gº©´š¿äß=¾.¿ã©<"?¾¿ç«S€Z®LOTHERsbg3FGL J0955.4+6940M 82?˜üw?®´}jvÜÏ?m
õ»ÿ+6?vìvÙ£¼]?¦ØŠ"a?¬ø•c»!?ëuzëP	?¿$]'g"ú?´ŒÊŠD•p?·´Ì	ŠA?¯Ž¼8-'•?ªE²ºŒ?앱-Æ?¦Ü×Õì›?"CuéÔ)?'4¹qÛw{?¶²6zc¿?£ðÂârŽX?ëu¯×ɀ?¡†4iÂ{
?º"G '¨?žIñ«¾?¤…Ùð¸¡?…›ñ©H ?ìÚ՛þMÎ?°Ymì'ú»?~¤ܝ
?wh‰šS?·?Z²|?¯o#áGo?æR씛á?ËÇÛ`äFf?ÆPmoˆé?Ç÷kW½?¿ÖÇÀ|#?µ&Â*•'?ëXwˆLÀ"?ª±Í…*d?™É5ý|"?'DÀL¬n?¾Ê0ö†É?¨Ù­A)?å¤â29¹	?´±`F"?Î35Ó\Å?²Bì½=?¶r'Ɯƛ?œÝߍ§o†AGN4FGL J1008.1-5706c?êAhX Å¿ï<Úa
À8¥1G ¨'À:,Þ¨@¿¿>™Ä@>	»j¤º?ľ>ÿðÈ?ÀÀáÜÿIø?ü1¸ðiŠ?ûëøŒR?í'ÜEæ"¿ã°¡óÛ/¿åº &5¿éÜo6ï€V¿ã{ÕctCŸ¿îës`OTHERunk3FGL J1008.6-57061RXS J100718.2-5703358?ºE[œç_~?°´N³ü£(?‰Røþâ|??ˆZ<¤…ŒÆ?ìR¨gŠ?±\ø?^"?Åÿ±økR?Ájº«Yô?¥»8ýVë:?£jKßb·Á?é$_ò?3X?ÁU]#­À?º&•Bø+?¥Bݖ»Ç+?¹.[¢±þè?§'±K{¤G?é•aê3mž?°"™V]?°§8‹ß2/?ŽàOÄ?©°A¾Ë´?‰—û¥K€;?ìPҗ^x?•à/iÊÕï?¤ïÀMÕ¤K?šcÇý9?'Ùtßö?'$]÷'ÐW?îhœ•2½Ô?Ÿd®Bx??°Þ£ªÐ´Ê?®{èˆ?­H/™ ¥|?°dQĄ.?쨐Ç&ß?µjPÉa¬o?´ÌLÔ?žÁÓ#Ÿ7?µMÜŒš@?§WV"Š‹à?ê¼À»Ÿn?­egö¤Û™?'od_—b?y¤[œR@?®<AŠõù?•$¹~ìc?튑¤Så?–‹Eyùï"OTHER4FGL J1011.1-4420?Ê7£^®%@#b'è},|À;2*߈'À<‰3úÙO'@ "«#Ú¦?ÿdž!Ðý?Î['ãG¯?¥ñïñêém?Ý'½†,@¯»ù9¿â˜éÛÑLŽ¿ìez]"/Í¿à¶@º°@¿áñ–`)5ƒ¿š¢ža:¾©¿æÜ¿· ìOTHERunk1RXS J101130.7-442241?îåÜ؀¹?™iσì?Q«="¥½Y?BÎü,È6´?¡،ñ
?˜Ía0í>Ï?鏄ˆC
¤?Ã,÷V¼X?MÓÖ×ì©?ŠÞ£T|…Â?ÈÇ?+Ë?Â£ßšÒ @?í¶Æz£?š €ÞI½\?qS¾aÎ@?i†D{z·¼?±9ÓKY)C?™qY€ò%C?ïv|T_©?nÀãK™û?@&Ç?q;v?+Õ[7j\?¯F¶–?n¬	*šŒ?ìò$
Œ–¸?°	ëȚËä?c:ð&Ó-V?Tem'ckæ?·Õ¼?¯Ð`Füû?ä¾z>N^?̓Ô98ìí?€ÙM>(H?'ZŽ#"Á?Õý¢Ð,±?Ìp¡íiê?ê‰8\à?¨p¸ ƒ³G?}©u™²³?rY'®ƒ­<?Äî£ê³ñ?¨!詳S?î!Pß/i¿?'‹r®ÝÉ?U¡>óh"?N÷y¸¶Š?­=èJn?'ÑÇp&AGN4FGL J1018.9-5856¿¤¶\"‰²¿úõ<WŸ#FÀ6*OÁß3À9­HJ­@øhÑz±w@rÇZˆ?•0£¥XŒ?Î_
¼òd6@6]3]$žE@/È´²¿ÊŸiKs¿àm	]¡Æº¿åyöÁgéÉ¿èàÓ¿Û¿í#>=ÓJ?¿ènq—òÐmOTHERHMB3FGL J1018.9-58561FGL J1018.6-5856?Š"~jö?•ÀºTVÙ?ë,'Ÿ;Î?ÈúA¢ë/—?Á¤ƒ¼|ai?ÈR¹'º|`?v͛yöŠ?"b¤ØÚ?ìXºÓ?µ
Ê<l?¾xfìW=?µúvÖC?²çþLz?¤¼w~·w?ß2çÈ?Ž$?º•=˜«¡É?ÜV3"U]?¹zMqI"³>ã` ÒÆ>àßY"Ènâ?í¥¸a°Ê? *8ƒl@?²×_;¾‹Û? 
Ú&Z:g?xҕ5÷%Ã?SKìÖ?ëŒÕ©Ñ??Ç<6µ7Ÿ?Á®°#–?Æýœt%§ë?oNÑn"£?~y›ì=?íqfÛ½fº?µk '?³zR˜EŠ
?µPp\"¼¦?«šÿr¬éÚ? 1¤Ž{i"?àÜálìè?»@:O(ª?܄æN~U?º‡ÑÊQa5>³U±St³>»G£€ÖÓ?í¥h°K?w?¤ÞÐ#f¶?²Ô§iidÃ?¤Þ½jM3ŒPSR4FGL J1023.3-5747e?ºÐjê_Ê¿ÚDUšfH3À7×xFÜ]À9›mjW@#_Jé2^@v¹<Íé?¶éπËf¿j&¶Ý?¾50¼ê¾@"Ǥſí(@éÈ?ïY¯¾ôòÜ¿ë[¨«¿ânŸð˯–¿ã»>U¦¿ÛþĖe×OTHERSFR3FGL J1023.1-5745Westerlund 2?cWøÑ&?iØTӉ…?E•æ"æ?N
Oy¡XN?ïçCgw¢=?n0æ6:Ï?ªÈ*ÐñÇ?´E%'Ðk'? »-
v¼Ð?¨hPtݯ?íGÌìÇö?¸îEàj?´éÞ"o—?£šmõ"û?«©éPÍ3? ˆ­5ž@Ÿ?ë¨2|æÚ?§Ü‰
[ø? ¦£ù\m?…–÷T•—?'¬*ªsgž?~'RD½ÁŽ?îh4jÑì-?ŒFÃçS"Z?r¶Cœ­Q?u;¤Þ֖x?P²ÙôÇu?T©+™t"l?ïÒ:x)ú?x5±Ë:¼?£ȴɧ¨?©pO¬è5F?¥F~a×KÜ?´$ÓPé_?í{kŽÌê‡?¸R¬j?²¸ráםw?¡?3lu|?¥?"Å"U?™YQØÕà?ìX-ª¡îl?¥uŽûûÒ?ˆ£ÜM$IV?wä%Äã±Ú?–Ÿ|
&Dn?‹Vzµþª?îèt®±6w?X†{pOTHER4FGL J1023.7+0038?{Z1ÀQ@Fä'úòÀ8Dœ¤æÔ¶À;ýÖ.u@ÿªó3=ð@Üb¼ºh?¡žÞÁ°¨Ä?Ç.95×@"2¹o!öË@½€šFM?·Y /_éõ¿ßa}H€!¿æ†_€>:¿èÅB>éË¿ì3ŒŸ`-¿ã'?´‰	OTHERLMB2FGL J1023.6+0040PSR J1023+0038?íÛ6ƒ}V?´«Ëºh?®®¿©JR?´ƒ3øøi?}ç|-Ôv?qRþ*ký?ï»bƒ<i?|ùôŠÕ?\EŸX·²w?dÂõ´}Å°?{=‹[ÕG&?wgôÕWQ?ídøbQÙ¼?¥yìÿ<ù•?¯£¶X5.?£—¶Ìw•Í?"‡3k?'Š8¥#k?ïç¨pL\?U
±™žË?U¦"ÖO°?FèŽ1Ã?[ü†l…?H¤y|"¿$?ì¶q¦¶b¨?³ÙmžÅѧ?¸I²öÖÄD?³ŠäivC?€þží×?u8¸Í5?ïMÅNíè•?˜ŸUÚÍÍp?sÄ1…?'=G:|º?''¥'!?•&h©Ê"Â?íU
IQ?§:¾DƒC•?°‡ö Y?£ÁçŒ-Ú¶?œUß
3'?—zqZ?ïÁ[¬?j\Ÿ(©áH?kuÔ2Í{?\ßÄIZç?q—?Ðçø?b
RT‡ÕñAGN4FGL J1024.5-5329?è¸j÷^Š"@
çDñ¢À;1#³co;À<']9—@"?Öê‡ô?÷‡åÂg=?Ö=…³:?ÞAãd¾Æz@	0)®O3D@™zu<¿ïÿþøþ"¿Ê0™Ã?ïÿTßUe¿Á¡;#—Š¿ÒUÖ¿á±÷(ÀéjOTHERunk1RXS J102441.6-533141?î8•Åúu§?«LQøaâ?tpÚu_Ÿ?r–nÐBý?©èˆNŸs™?©ò@1šî?éŒ1{(?Á'¹ÿ?€/Àî' ?Š8ñ!搵?ÈÌ>ƒaì?À=ï5Œ?ì
Ù¶?B?¥¼÷ôlÅ?'å°Ä9‰?ÐÃsÕO?ºÝÝAG?¥!,³WÔÕ?í½G€ù?LayäêÈ?qP3uÏ?\\,"ÁDW?±ÀÍà\?ŒŽ3½zR	?ì:šS0‡:?´ˆM\xS?†4鵞"{?'ѯˆ4í?»d/Z!?³S''±È%?â¹IÏE¼¼?ʍ`4aö.?""U†ð?¦øβzó?ÙT'	.Qø?Éüùî̄†?é•]¤×M?¬~ŠN™(?•Õð˜÷?&ôéÿì?DZ–«?«7ç	$q?ê˜Ì.Ž« ?¦ÿ˜v	ðº?zÑy_7¬?tXo†äHß?ÄÆF‹T²_?¦ê1†'¨TAGN4FGL J1024.5-4543?ÄÃ|äN–@#Àd©ÍÄÀ:´úŽ¦÷À<qZ»7y@ êÈÓmû±?þ"ä0—?Ä0³|Õ9?ªZÝ#å•ú?èaþÂé<@_£Ùäbk?ïéè »6w¿àN¦@Æç€Ç¯;¿Ô]´;0'ª¿Ñ¢5Ÿt$¿ãµ\"•¬$OTHERunk3FGL J1024.4-45451RXS J102430.1-454401?ìzqQ7;g?Àn‹iô?~­Û¶m¼{?¤"m™}Ãd?ºA—ºqUƒ?À	£À—'â?è?|˜4I?ì{7r¢?}xž^¦?'+ùT«ƒ?ÎI'	K?¸i¼9à)?íúˆQ¬y?™0²'ïƒ?rÇéãYéB?mã|`ֈþ?­þ}¨Z#M?˜µ¨-Y<?îµ	S³'Ø?}²¿3÷É9?r¹@;Lè?U±'
6kH?¢XBÀ§¢?}"°-³2?ì4ô\€?³áž4ƒÌE?kŽŽÀy	³?mçøÄû?¾™ãè™t?³ÊB‰…x?àTNÆ&?ɯoÀhv?ˆ¯ª÷Ík?'vêžî
?ޒv
"yˆ?ÉÈM¥éù?ꥆn2|n?©¸ð•â|x?~}/:¯?qØ{±?Äuþ-†º´?©TŒ‹sy?ëüD"F³?—
©]N=9?‹[SÆ§š?z&Áã³ù?¼²pô'Ø?—†]w‹o
AGN4FGL J1029.3-6657?éÈå'tÀFr*rÀ:…úcÞ̪À;ñ讪¢Ö@ŽöÑX!Õ@WWÂHå?Æn=à¶8·?šOãÃ?Ø-™–>›F@Ï#¾Ì?ï
–V:‰¿è¸…íë*†¿êŽ
>¬ãù¿Ý¬ºÞ¿¿ã›â´•žb¿åPT "žXOTHERunkPMN J1029-6656?ï–tžëñ‰?€:½#.?QÙRð$"1?G_iMï%?ˆ'­ÚHX?~в–ðo?ìtÃ,ºô?´ˆB8œš#?Vˆq¸5?`Âͱ*…<?¼€%1ñG?´QÚö›:?îqÛñǜÑ?"V¡>¬ù?tþ‹¾{ ?pùn!åè±?¦Bo~L'ÿ?"ƒ‰$ˆ?ïyZŒ
a?i|g"át?P6üw$›¶?1,[Ûáî?¢}o¡¶d?h'>2ùþ?îÜWùÞu8?žèc:¾Á?e@£±
E?`:l[÷ŽI? æv&ƒê‰?ž"'zÚl?èn"¿ƒýÀ?Âg^Q!¹A?aUg3"‡?rÝ&ê®?ÎWd|°?ÂA "v~?ì^¶ۅÞ?¤£Ü…Õ×?ˆ#?˜Y?Šqˆƒqº?ºîŽ_÷?£-Ø&Õ~?î[u;ì?Y?†í©ËœÊF?jV$ì÷Ï*?T;/–{™?¨£Iô$[}?†E«øAGN4FGL J1034.7-4645¿î3U—k±@#Û,B»fÀ:ïùZÊPòÀ<cÐÜ&$@"pçɨ@'}ô!¥?˵Ï_‹+? ¿5#g'?Ԇ$¼øÄL@¹9õš }¿¿'£ê¿ê±(+˜4¿Î§!—¿æ]gÿî<¿ÊçFu°0_¿æÎbß\\OTHERunk1RXS J103438.7-464412?í±0£z²½?³ž°š<+Õ?Sä_Î
QJ?BýŒøýæ?²&écÉb'?³šn˜™?í')Å-?²ã¡¡¤È?p# ×$?wöSV…È?²ìÉӌô?²@)©CF+?íèŽ'†½Û?šT HðX?rÿ\à4lq?p'ÅÏýã¬?¯1ëw—B?™jøÖÇ˧?ïnÄd&"Ý?jJv·:–?C$ÜwŸ}?/kèm@?'ŽÒTñÕã?j]]ªàQ?ê㻧>%ˆ?¹"W–Ðø'?eºÿ:â?X…\;»P!?Ä)%WV?¹x}%€Ô7?êHojœ&?Ä>R\Tzè?zë^Ӌ?‹¶Î«º?Æç^ã)?ÃУñâ0?êÈhPôB?«j÷ŒíMq?€½}"òmH?uª§Î¤¤?Ã҆âª&&?ª¢:VVè‰?î.MpÔ±ü?‹#âEJ†
?Vá'Ói
'?Jѓ¨Éàâ?¬d`
$ä?Šûªxž3AGN4FGL J1045.1-5940?"߲úàÿ¿ãüpÿFœÀ6høj	‰À9êƍîj¬@î«Ä¿b@©²=ÕM¥?'Šg!¢<*?¼Ø;•ØCù@'Ú^±¬@¿+½óëö?ï(Åñç9¿×q10–v¿ãì2žðÔ¿äTµÏZEÇ¿è°&äpX¿ä¹Ùk€,OTHERBIN3FGL J1045.1-5941Eta Carinae?৉ªÊT´?ÏҖ+a=ï?¤CüÍ#<y?©ü}™§¿?Ü(mP_i?ÎTM&Š"?«‹Ô‰)•î?¸ÖBµV??⺕¾åü?͑€'zÜ?×FCA"k?ÉXƒ"Œ©
?ÕD›°@?´ÙApw\?ºÆèk?¨Pä?¡?âîwþz€?¶ŸK/¢[¿?–3[_<Ë?ë©Ø;Jñ?ÚS†`'øý?°ªy"*>Ï?â$¤<éH?°-'Àç…C?Ù	È+äp"?Ð+;Œ6ôM?¦ÔÍz±Fë?¨~¤X‹ó™?â
Ï<¨?Îã¶öC5+? µ>&0ŠD?²˜^ŠÖ±s?ãŒîÎ)n?Ò*úeÈm?ÖÑ]/¨\?Ðmû`?ÖÌ%N'?µºˆ÷ÔÆ?¸° 'íi*?©lñ]?áܕÛQ¨r?¸j[gª•2?uV[`Ä~?ca¥c0¹Í?ÜEI*–V™?¶hÂU QŒ?ᲯNP‰Ê?¶Hh3©MIXED4FGL J1045.7-6414?çIiÞôuÀ'C{À9Ϻ˜í¢/À;¼áG®{@báK´ß@"õ?²w?Ã>ZÕÈI?Æl–\ò@\,CTéf@裉1—}¿ïþ¢˜›Ã?ïúiˆYÖ5¿ã÷M©Öþ¿áJ·~†îœ¿ìSá~Š ¿èú˾!OTHERunk3FGL J1045.3-64141RXS J104537.2-641438?ë
‹z-SÜ?³IwHÈ?"wǕB?‹¸Æfžs?Á:ñ!?²Ã©b!xÅ?ë{e6n/?¹‡ãý—ò?v͆ı÷?}d@0n -?Á[am¶ÅW?¸‡{‹Œr?땶Ú?¥_«ãÓa'?¡&êfÅï©?–ðaG?º¾ÚŠ"\Þ? ·ª8¾±ƒ?ìoE_õM?‰Ñ‹Ì2? *9¬¢t"?z‡C <?´r!féT?…VFÙê?è4wÀDÂì?» eï•?©ä§wè>Ï?¡sbé¨Qx?È´÷ »êÛ?¸êÎ9"OO?äíKu?ÈèëâøÄ^?;§õº/?¢åÉZôh?Õ+'wd?ȑÃ}Sùã?ç®ˆ$bq?±®t——D?°O^!ž`S?Ÿ@Kÿ'?Ë¥–ΟF?®"м$ñÂ?è"
Gó"? †R}ÆíI?°ÖWèñ±ä?"àïz"óQ?ńªðÀ-=?œ'œnRqAGN4FGL J1051.6+3253¿Á9íü66@OÃ˼+"ÙÀ;'?Ï"èÀ<êՌŽï@û´ò»sß?ÿ†YJôðØ?×ǘšëÿ?©	%B¯¨?ѱÁ"õxh@BÜÔ+æ¹?ãxo'Á¿ïÿôw5Áƒ?ïýއà3²¿×E;ÿ	µá¿Ô—Ø"¿ïÿe`õäOTHERsbgNGC 3424?ïÖ,ÿ+]–?‡;Nü
©±?4á%ª\7³?GŠaSym?s›n(Ò/+?†<,<Z4?ïì=¥¢«?iPЃ4Û-?/þY±$¶?@@åN´?aÃîG«ñ?fÀiÄ­?îϖ²£D­?™tH¯ÏÅ?M"HŽWi2?`tsÆ©y?¢'°¸D*?™t³Êâ?ïò2'²ø?A—ιÇ–?—fGÒ?A°rì"˜?Zr\ã´X?A0Y—?úi?ïÃö(vþ?ƒËxÙm?>ùP;@
?HvëÓWÈ?|ˆp7NŽ?î'X)þ?ïºôQR6?'³/]?Bq?rl<?T^gÕëÍ?€ä§|ã®?€µÞGkGû?î6—IïH‰?æœÕZ²?S¶#"!
?c‹ž²œÅª?«øÚ§îÖi?Ìeø!Œ?ïßU¹ÇÉ?_¼c3¼Õ?ù´…j?ÒšN†?o⿼9ÊÜ?_P‡sӔ™AGN4FGL J1059.5-6021?ì#%Êûøp¿Ü¾Ò
SÀ9³9ä'À:š>—ëC°@lTi¹­
@ªÂT£Æ?ÊäÑ{]C}?Ï$_ZÙjj@>ä\5Šü@2\sž]?ɖƕüA?$Ç/¿âa4x­'¿æ¥'ßæÚë¿ïÿýç!é?ïÿ·pD5ºOTHERsppSNR G289.7-00.3?ÝWË`á?Æý›»v§ì?ÁƒƒÒ ãi?º?Êtœ£Ô?Ùæ¼Kj?Æ_ÝÅ1fÄ?Ò>Àj†˜?ÅäîŠ?g'?«æD	s?¥…0GnÊ%?å"7!v¿œ?ÅRUÅ%ÛÔ?ÒV¤?B"¬?°c˧¬Ùr?ű ª
?©þL¦€?áóhsö‹§?²tàõ?Ò&k¶ÔµF?¬B"2µ|?±ÿãlÏË«?'.^l"Ô	?ä¬Í·iŸg?­":9I¾3?Ó)Ր?Ô?Â¥­ð	?ÄDw$
¥?º9û±35¯?áZYË«î?Å9ÃÃí2Ñ?»'7RQ±y?ºk§:cv?±¦$B?±ÞÜð™J?êm¤PàJâ?À{Ÿ?˜=Æ?Å[êN4bÖ?¨C9fƒ5¸?Äû³Às?°e˜¸?™j?塆'än?³Ÿ'G*?· ‡Æô Å?›QÙk/"?·<Ml:'þ? yu°?ê$eYÃb7?¦æ܎þäaMIXED4FGL J1114.2+0638?Öiªþñ¸@M'ËÿGs\À;¾vÌ7«À<Ø'QT†@"_©mø,?ÄWoRž2†?åÄáçDò?ïûo! ä'?þ8¸É	É­?ø2¥4M¿éç÷Ë~4¿ïÿߞ¶Žó?ïÿ.´Hq‰¿äÑq5Í?ʌ3)£'¿ìYƒ)Ì@OTHERgalIC 678?›"I›?®	÷ˆšë?bx'|a ?|üºæÇP?¥í"ØÆ¿?­³`^øN?ïl
Öh"#?˜3]QI0¼?rÆÉƼ¡3?…ºD¿4¤F?‹™%yêÍ?n€V˕u?ípÁÅBü?£ÒFU¹k?ŠŠóqMád?‰Ñ•õ¥R?´£"t?¢»#§Ø?꘮Á¸¶Y?²lWÿß1?U"É4[6;?SRÀC÷?År;fˆu/?²l!úßV?íÝڜ]?²†éؐµ?zÆÿoGQ?Šñ0¼éÞ?®ÕÒu|Z¤?±É"§ûÖ?î]¸áøõ?®¦áš~	à?…_'D'Tw?–ëUOÇüI?¤Ì5'•?¨Þ™¬M¡?ì:ßÏÞÐ?©1	í|‹:?‰eéÚGáJ?ˆÔTÅC{?¼©kÅ\&X?¨mj"ÉÞ¥?çW­š"Å?ÁÒ%=ôy±?AUçäm>°?TZH¶`M?ÑGû	~·t?ÁÒ
Vù"ŠAGN4FGL J1128.2+5831¿éè›
`Î@K¶-VÀ;b°+¬VÀ<ёúhçJ@Ó£åLöS@îÛŽ,?Ð{uâZR²?¼oa^®?íÝe k/y@Öm¹kñì¿ãPxˆ§ÙοévýÃÝé¿ßäY±L¿âmf4è?¿ëўJÙB?Í×͜U‹£OTHERsbgArp 299?ïÆí> :ø?m÷TQA?TK~´×´?C—cS/?wv€¯Ñ¶	?k+ˆà?¶öC5?Œ.íCÞÓÀ?_½y'€Øí?fpǟ­Å?"ßc>Ÿ'?‰dÂ[á{?ï^šéꃱ?ƒ'4.iK?má³ë}² ?nM…!Cì?plKC$Œ?5)¤án?ï™Å¶xÅ?g·?Qæ…è?bD×Lüt?HŒ¶ÄßN?"ý†SÑ£?fŽV~–¥Ë?ïw溬?"'¬c¢q?cw늯FV?TY÷íµÄ(?^Ëjá›?ƒ†ÇgW±þ?ï5èÉú×Ä?'L
*âgû?e?!%'Ü?nV÷†%rÒ?–›šýx?8ž‡Ïû?îÔígØE?±ÐžÈÀi?sìÄNM×?rqmvr? 3—DZK?ŒÕž‡þ?9±–T?‹Î=¦ƒÖÇ?wtRÅB<'?fö­(¿'M?£…ò–I*?Œ}úm/AGN4FGL J1151.4-6248?劸'ñ~¿çz¾ï>'À9!JÕh-À:À´†"éß@'éçÆ²@ê²ái<?ÂøScTc/?±¨Ã
†P?õ§ðª!§@²™Å¹?Õ-GáÀú²¿ßø€‹*Á¿ê¾9÷r'Å¿ä"ô¿7G¿æV‰äð°¿ëaÚ`3F~OTHERsppSNR G296.1-00.5?ÛÁîÙ"VÓ?Å"ÈJÊ|?œ·™$wÛ8?'a4á#¿ú?á9KʝŒ\?Őpe˜¶?ÒèÓ	
+?Å.À$üAb?–|`àÛò?•a;¹|~z?å׶x€"?Ąmk	¤?Ø·ààÆ?´PÎéàî?²iÏþïø? eÎ*¹Ê¹?á¨ê,┾?´6}ûºhJ?ÙwâÒ?ñ?¤ÈúDÕ'?£r"]yߓ?€•.Z¢?âå`íU®?¤ö}ã?0ì?Ïlo'½÷?¾™Çãj.X?£ÍüÐ/3È?šøÙæ¨Ðu?æèNvä?À®t~úSe?ÂK.dõ֏?¹–yfŽÎ?™€­k[äD?¡Þl1'?ê¡.ûYìÊ?¹h,C'Â?É]w25d?ªêËN=<Ü?³½SⲨ?¡
ÞMÉN£?ç0÷·1/"?®a&èJw`?Ä9üæp? UÄQ~?¯74ÈÕ3ˆ?'v@dyEI?èþ
y»,ç?¢(…nåOTHER4FGL J1152.6-6207?å÷u #È¿›N(¾ rÍÀ9ÕrQV3éÀ;€ö4¥#@åQ(À@%iF·G?Ô: $x/g?ä{àK.Ò@Rµ¼åÎü@Á'kՑ¿é%÷@=ݱ?®T˜€uv¿æbÀi'¿ë›[Õì¿êC,oʓ7¿ïÿü¥¬¨OTHERsppSNR G296.1-00.5	?ЩôýåÁ?Áîëðÿ\?À¯IäÐy«?´Ìkt{o?ãÐXŒLîµ?â_䟯ç?ËÞrš.óf?Ãâ-k6ôx?³Ü‰Ì½ n?«´
SÉ­?æŒÒêM‰?ÃaN]ŸÝ?ÐoÕ69F?¯™|ðïc?Á—QéŠPY?§¶?É(.?ãb@ê€çÇ?²½×a[?Íu¸Û£?¢`ОjC?Ä}Üy¾?ŸnÁäj?ãƒÝY•{?¦ºfY*‡¡?À–Ø
›?´ÁöÈp]?¾c_ö?´WpèëÿR?èݑbŠÜ?¾ÜÿŠdG}?³¬"çÒ8?¶kºGRé¡?ºÍ€«$ö?·½9ޔy?ê0Ì×ð¨…?¿vúeêÉ?Á²(q8Q€?§¢Y;?Ân_ÚD?«ø½®†A¡?æ÷Ýí0š}?±›ÏE¹LÜ?²B\öû8?'åí±Ô
õ?Çåaׇ«?«*F	×R?ç¾\ǝ?¬Ù^˜¡(OTHER4FGL J1155.2-6259?ÑçÅb0‡î¿éè:ÛÀ9'6TOãmÀ:—yóáäŒ@"éµæ¬G@¸5u-?òƤ^ïy ¿îL?á&£7¨ú@Öð<=ž?ß¾Y¢2ÅO?âKÕážk¿ç˜}Ú÷1û¿æ/Y‰ß¿é«^½ûx²¿æÓ¾ŽE¨OTHERsppSNR G296.7-00.9?®=C45¦P?¯ÿÕʸ¥—?Ž
à§ÌÂ?­páJ?헻u·g5?µT²,4&Ó?ºwö~#?ÀykQÁá?•ä!¾pÝq?¡ðîWE"?ìà!é3á?Á@zhý?΍}Ó%½?®=)Ü?¶ñ1‹1Z?¤péAå?å›âe §Q?±ªèå³ØÈ?ÊCšš±®?°|1W½‹y?€(×Әµ?€Š†,«?é:‹¼·*ú?°¦n@ä?ª
`'Öò[?º¿ãMu\V?"'f^IZ"?²'fªIŽ@?íÆÅ	U?À;²è ?²ŽèoG?¸¨Är\Õ?"ê‹Å ¨?¢úÀ~gå?í i›¾Ò?¹‰ù})Ø^?ÁX¯4?¤÷uÅc}Ò?µS4h9?£¢9±i©n?éîÙ'Á?­SeµiîV?¼s:c—î¸?´:Ÿ™ê¡?{þ4Íñp?»ÕkV?ì9œIÞVž?´¼î;}ÄOTHER4FGL J1155.6-6245c?т88º¿â'óøŠÀ¹À9+û¤P¬ÁÀ:lE(þüË@Ö*%mwÓ@íÍÛÀ…—?ËJY™??Ñäg¾U:Å@‰óžÈ­ƒ?ö'ÞÉN"¿ç€E4½vî?熁žü?ŠºDΪâ0¿èÒ­N ¿ëfÖ-¿ïÿõEq#OTHERsppSNR G296.8-00.39?¥¦Æ	Üo$?©Š_¶º?¬<·+Õå³?¯TÞnF?ìáÈ,²™#?·•'%z1 ?¼ÃÊ*í$Â?¹°SÎ
ÿ?Â[Ë®99?¶øàdaÜò?çГ÷vÍ?¼%eÀ#F+?Ã|¬-Åàõ?§'±]yŒ?ÀfCI%?¦`9EƒÞ@?çD"Lc¹?°¢gò£88?¤âÚ]â'ä?†$X^m?´#ށ€?¥ózêåŽ%?ê/¥Q*6'?§pp¢±D?š$þúâØÔ?—BQy¾^ª?¬D)œý?®^
#ðn>?íj5Æ(?²ÛcîóÛ]? èqR"…?¢73A!¾?Ī/"ä?½œ'ŠpK?éÆí	ƒ6?¼§@t»?µrÙ0³Q&?œ
kÄl¢?½Áí5MÚ?¥ômY,"?é™g2û;0?ªö	‰öÌ?Šç†3 Ãä?w¢«8löÖ?Å
:ý"$q?´S"%&§ ?êQÓ'Àõd?´0€¤ ÌOTHER4FGL J1158.3-6232?Ÿ±'gSÔÇ¿ÒØ>e@v"À9)Þ®v pÀ:½¨ö-ï'@ XQÀ'ô@Jh˜q?Çm™I'›?Äug5CXÅ@nÜV­Œ@»{–¤G?î"ßÄK¿å´—1š­¿æÂB/Oy¿çñ§w¨®¿ë­ÌŸJ¿éë֙Õ)OTHERsppSNR G296.8-00.3?æžf]8?Ä´'½Ìµ? Y¯% b1?•Ôë̎°Õ?ѹNvtj?ÃØßIüù:?Á@¿§?¿±QÇ? ¹G\P‡? @›̜D?걛Z±HÚ?ÀKjȱñ?â`ö©®Ô?³çè<h1?­B?Œâñ?ê<pßì-?ØHúªÖ'Ù?²"1½û?Ór¡~{—6?¨žq'‡é?«Ó½È,g?|Çl^Ï£?ä‰}•.~?ª'RL d?Ú_ˆŠÂU?Å
K'¡?¥ó¸1?œÆÙ\–ô?áq8½"S?шb\
?²	¦ÌŽâ§?±œŸ»-|?¡ɸlÙÍ?«7àìg"?ì­.Š¾¿?µäÃ$¹e?ߐ› §LW?´Cmý"[·?®Ì¤b9Iç?ŸG•Wúïž?ܕÏ҈
?³o8$}ß?·ÌxÃPÆ?š'XÃE
?´ â¿üz}?¢Fß¡vï?ê'c9,¾Ç?¨^ÆGÃ%>MIXED4FGL J1159.3-6122?ÂGÉ|O½?ëýH•›À9Öƒ.ô	À;šCㄟ@Jö‰‰¬@¼*`%څ?Ì)ž‰îUß?ÉŌ§Ük@_î¥d¨÷@dHÔÛ.?æüóÁ-\Z¿Ø¶ßz¤`ó¿á-ÆwH5ú¿æQ6É>£¿î	¡Ñv¿ïþÙú²¹%OTHERunk1RXS J115843.7-611934?ÙO=ÁgÐ?Ä{
!Žp?«?bÍqæ·?žÈ[¿º?á¤jò«óR?Ãç®ÛJô?Ò(U³‡?ÅÆ®÷5k?¢²®hˆª‰?š¬/t6ß?åÀª•ê?ÅìsA|]Z?á[Jû6€?³]Ó="Ú?²v‰~UÏ?ŸªuæµKê?ثǪµ1?²åªñ.?ß-:ö¡?¢%U]U?¬0æéà?"èP£ëÞß?Ýu¬§4Ú?¡gY'$l?ËíŽ@þ?¹zq´mó?°íËw.­	?¤¨x¶sd¿?ç!‹-E2?½§:xï!ƒ?²•GÝ1?¹Åã¹ù5‹?¤g²P¹p?¨Tãuõih?êꏈý?¼1.q鍉?ÒÍSixXp?±7Á…˜q+?¸XÇîöÖ&?¡®`L²:?ãŽ=M'd?±ç
  y ?̚¡R0à"? ¸åÿ¦*?´&VÛøÇ?—Š§~ؤÒ?æYRà*UG?¢•xP³MIXED4FGL J1208.1-5149?åog¼|È~@$ô‡Tów\À;t2À<kAHŸ¬@ oÔn+ן@.Ʊ?Êœ§@ W?¬éᅖ'c?äõ"FK=ì@9ʎÙø?ïÿ¢­>'¿é̱‰zg¥¿à˜Øÿ`ö¿ÚJS`OK¿éÃsݝT?ÌtÀÇ/ÿÍOTHERsppSNR G295.5+09.7?ï	kþD®?ƒs<Ö|¦R?Xఋ£å?b8i^V+?Œ¼Èõ\ ?'gf•S?ëèìߙ?¹§úZyž'?zìb8Œ=?'ïâ:š4?¿Â|ß%?¸ˆ‰ïs?î½}ˆZÇ?Õ¬¹>Í?o~À£<f?nfä%ZØ?¢<@7¨Ó?ŽÆU5ýÃ?ï3ÞË
@A?töy¡[?d [½²|æ?DÔfP¡í?—#ŠT?sMŽã`?îhcµËÃ&?Ÿ‡ì<›€?p	˜hï¾!?zH¶%Ÿ?§x'˜5™Ô?žDIÊ7Ž?æÖåÃ{º?É,ˆò`I?/X½nP?Ž«[_‰_?ÑÕw…úù?ÈÂGbÀ¬?í<ÑoÒS}? $ž¼`qn?|0­ˆ–|?{×N,Ÿ ?´Viª¼Í=?Ÿ)Å4ø¼1?íO\¯¶ïô?"gi¢"E?{Fcì?fÄ=~ˆ«?³ÍªÀ?"*ˆ™àôôAGN4FGL J1208.5-5243e?ßyðŸS²@#0FÜ]dÀ9#V›‡À;ŸâV¡ÍE@ eSµø ?þÙû‰xº?«¬=
LŠ?"XÖʖU†?Üyb—yÚ?øˆmÅ*l?ïõ΃†1Þ?ïŠIˆà¿á÷=^ZS^¿Ö&Å#
F¿àêâ«¿ØÙ	Üwº¢OTHERSNR3FGL J1209.1-5224SNR G296.5+10.0?ê›k¬Tþ?·(4€Ôën?ožÑ³Ü¦ã?cQ-0›‡?ÅÖ	.i?·#¿¸è?êK7h÷æ+?Â	ÑKGã*?"®—MQ&?žx{®ûj??Ä]OsR)?À"û$N?è÷Fo>ëè?®p!ò̙?"fzž±ÐU?‹µç ;3?ɶðåäT?­\TCíù??é]|w'Ò?¡çÉÎþq?±CDÜC†?'&AôqJ~?ÁèŽU²±?š"~…=­e?åÒýCjÁs?Á>dOñëü?åPa_V?y4Â!F¥m?ÓÊÚöƒ`?Áè'§?äeq¹"Bm?ÌÿáŽÈ&Â?å ÊÉê?¥!ubÔ°?ÕV˜S»Ç?Ëú~ý5l?çGIàâ?°púšvŸ€?™`6÷bøs?'Ûý¨s?Ï·Ëø€Hª?®ÐÇþv:?äjòF{[ã?±¶g¦²zÊ?¿Ù›|Ȩ{?¦$Ç¥9˜¥?Îgi'®<5?¬È—mvN\AGN4FGL J1213.3-6240e¿ï¹@󇙿À=çՒïÀ7@)íÀ:,…dž@™bRZ•Î@¨]Ywj›?¡‹:ÜúA?µXè_¶…@lâ¬2#@z$b_ñ'¿Å¥'Abv¿ÕàQ<¿ãyâyÝ;°¿äv†¤ÊOD¿ç#ĀM`¿ãhë¡y6ùOTHERsnr3FGL J1214.0-6236SNR G298.6-00.0?‰=Ën|*5?"^xž[Ò?ŽÈñ	½Ï÷?Œ
îóª¡?ïåHSg?'Ú—hŠ6?"PÄ~ú¥Ü?›Ê¹4/*½?Ö¦E¢äú?ÆÉê¢Ô3?ä
WX›;t?ÅÎÆGÞ¢?´g>š	?¢~÷ZP?µZ×vzÙÜ?£í²õ†
Ž?êÐø)‹®c?ªt¶F‰¸a?¦(™¬Wïþ?"Ú»}
)±?ÈgVj3¿9?¢ UKœ?胠ËÑ?£øœ@_c	?Š‹ö\¬íù?ƒƒï '?"7\'ª?¡±2jõè?îü‰ù,k?"‰þ"©ì?Š³²%áû?›œ‡ZˆÔÔ?Վj÷o¸ ?Ésýх ï?äÍû»D0©?É|¾[^º9?°Ý‰n׎?¡'×ÞlÀ?µË		[Kë?£·Àl´a±?ë*þMoÁÑ?©ºrÕ:?‹šüÌÐÚ?r½+FŽ/‡?͈†£êø©?«žŽx·7?è/rd݋r?«²!"U
¥OTHER4FGL J1256.1-5652¿Ù‰hôá@ùú}	@À9Ð)é•öÀ;¤uÓÁ³"@/=;tË.@"|tÅ¥?Æ-+²5qÒ?àD@÷–û@{xÎø?ø=ìl¥DÉ?ïúÂT£Æ¿Ú%›eK´3¿é1¦€²Âà¿ëxöLÖó¿åŠºÙ…Aô¿ïèP¶Ñ¸ÅOTHERunk3FGL J1256.1-57031RXS J125554.2-564945?ÞÚM£ô?Ŏª²Ï(?¤6Qh+?ŸUµe¾Oû?ޞèA·T?'n¦"°÷?Õm¿[J(˜?Æ(Q)9?ͤ¡<v?Áy	ðÞhÅ?Ü
nSØn?ÀͳHA?ä"F7‹¡M?°¨¿íLfc?·ã漜"Ú?¢
Ê ¦ó?ÐàyáÝ?¬†c6$7?×`Ç»•í¾?¥¢þMF†?ÒOA'gŠ?¨ž™<4`E?ÖOöˆ4?£¹ˆ"S?ÔóR}PbÄ?Ás#B}?°VGm#…?­Ê%4K.?ル÷ü6®?Ã<þÒó?½û%…[Û?º30C"ªG?Ön­&7?ÈJ2Âä°]?á	I(N9?Ķ5Pﱩ?܀µ,G0Á?±iKT.ƒá?Ä{V©k/	?«"+Jp?ÙAŸ7º?²6Iˆ¯ó?¿¿	!=?›áú;{ô?ÛÆù€?·hÞö!O?Ý
w¨¿7Ÿ?´ÕŽ2ûXeMIXED4FGL J1302.9-6349¿ëzð5¹©¿ï"ÃÀ8Ôðý-½¨À:Rj¢Ž5@;ó HŸ×@#v"Á›@?µåš¡+‰¿µý 1
i@\[›1IN@î1·?ïÜ<a/Dç¿êUÈßWhó¿íÉÂVQEm¿àÚ!2Æ¿ædÆ®0*?¸iE~d^úOTHERHMBPSR B1259-63?çu˜N§?È_þ9Î¥6?Xîîy:??]âÍ¹?ÐüèLÉÌ?È`¡‰Z»?í?ÏßYtï?ˆîâ²?X÷Ϭf€?€ iˆ?µ¡ÅêJ?Â8õ³;?âòõ–çÛ?µ©‰È €.?¤xÜé-3H?šÍò(áQ'?׌°w¬‰á?´D÷חŸý?îAâb'£€?•¸ïäî›m?1 íþýà?!iá±e‡&?«¾—ùÞE?•©Ó÷¯´?ÙH'ìè\\?ËE'UÉ$?aèЮ»"?caø?"¶Ç?ãI͸ýY?ËGRhÇXˆ?êÎüÂ*SÞ?Ť@LÝd†?_†>z9"?;5r%?ąz¤6?ň‹ûÝ?åìx—Iò?³ü'J !?žâ}6'53?–w<‹¹—?Ò8æþs°H?²röˆ+3ë?ê•H÷ëp?´{9ßA;?Pê½/lEv?Fjñ¼«TO?'nDû7?´tN€àrîMIXED4FGL J1303.0-6312e¿ìD>H¿ÖáU…m'«À8EñÓò[À:ҕˆ'á@"'|2iµ?ýÚ8
2ˆé?ªO"›Ø¿£e">=¨W?÷ˆ•âU?ûÈúDÕ'?ïh«…Th7¿Ø6rûé¿àÛ?÷fÔJ¿â…`\a)ç¿Üíaw¤Q¿ÃQu¾sÐOTHERPWN3FGL J1303.0-6312eHESS J1303-631?¸ƒ	îÂö?¯pUVnj?y5¨¯ea?pƒ8+Üüí?ì½3pßò?°¦õ–¨J?­ÄòÖÕAï?¶
±	Òے?£ùBލC¿?¨"œ¼Ršñ?ìä¤rÝå?¹Á>/2?ÈV_Æ	d?±Ämþ?¨Xø˜\š?šÄ²ûT"?èdد"?²%±Ì'?Äà(o"?¤;"ìë×þ?±Éú€ ?–Ù?èŽ×\®èÇ?©j̤]?²JÔÙyÝ?¦X'f´ë?ƒ"fÎ3ˆÒ?z•"9Møˆ?íh"ɏÅI?¨T:æÑ? ï›jy?¨+f9üÃ?D\:
y?¥T¥þª?î&Sü¬?±dPI¼š?º
ãB…
Á?¦"wo÷;?Ÿ'ÞÉ·_ ?"yQL9C·?ëÁ¬¡ob?©p	0?«³"!CcÛ?"d{VlÜ?µQQ3"Ñ
?¦4–v§?뚝—¢jñ?ªÀaƶ·OTHER4FGL J1305.4-4928¿ë€~ˆ ~@*«h'0ÆqÀ96s¾=½ÑÀ;üR$A@Ò@VÝ1t@êù>?­7›!Ùïu?«ì^Ó¶²?üuÞß)@¥^¿þÞ?¹j£Œâ|¿Ø¾U{1¤"¿å™ç'Z¸³¿á¾'¼ÞB@¿çpÖAj®u¿àâ~å¹-OTHERsbg3FGL J1305.4-4926NGC 4945?ï@ëÛ€?… ½8{Á?jþÁ³‰oÙ?Z*¦Èo?"êSsÚ?ƒh¡À^ÉG?î¸u 'EY?¡J²ýʚ?Ýï›)>?"¦qCd-Ò?™d–:P?"ti¤ØhÂ?îDZ;Ï}Æ?™!K:w0t?…¦áÑwɔ?ƒыH¬?¦P£Ê^®B?–\«³"Åß?í§ªÚÅÅ?ˆcÄ<ÞÂ>?ŸX¦GB'Þ?yÏ¡…ü¤Æ?¥Øÿ3r
n?~QìëÕî`?ííöð".p?U'—ˆB?ƒFµ'¼º??u=ñiô?¬NãrSy?›b¬à'¾?ìµ%]ÌS?¹¢Â'ƒ?¡ØÞI"!?°5sc§?±k‡±#sÚ?°/Vÿ?ìy³&L^Â?¤;—«Š—?–ÄÔ3]?ŸùB<?¶ªõ™l¦?¡zÍL_»8?ê/lÓy?£_ítŽÒ?´tÎ6˜é'?"(Ë|õÝ?ºË,Â3t?™¿Où%AGN4FGL J1305.5-6241¿ïz=]P	¥?Á9Û×À7Ù\M}À:\Ê4lW@xƒ
¼L@ãö<1ßv?­R°Å/J?¤§Q"¤q?öéëÜ\ŒÉ?ùÒ¼­ð¾š¿Øž½ûx±Ã¿Ú)²ÒÛ¿âþtàÀ˿㕮Þ]¿è¨Ÿ%ʔä¿áýiíÚcŽOTHERsnr3FGL J1305.7-6241Kes 17?£/»Ø©fü? ¨H¬=Ìn?šЅ'FV?™Ê õîÚ?íü;dT=?¨o¢jÇ È?¨¿=çð?±PîdÁ?¼¶À±`Š¯?·uššš?êÝ4}ë?¼'-"Á?»–<ž‰?£ü*‹Ùbh?¾€'ú"Â?©Ð~Oi´?è̈V¹—?°bâÎ@ë-?ÁÅ
Õowv?¡L7wKÍ?·ÏXHo8?–VüV¡N#?è"ч¶\?¦=å
ÂR¤?œ‹<"‰Ü|?—*oVÓ?œÚTð~J?ŸpÔ¥àx?î4Ów>ƒ|?¨­Á,É?¡+£×<Æ?¢DƒÍÓ©?¸2¯R.E?¸Vâ«T"?ëæïØaø»?¹"¡Òo›f?·~áÇm­Ò?¢õU9;
?¿»[
g¸?¬œPÃJ?é/L[£>ß?±0ÒöPŒ‡?«—ŒnÐҝ?"äŠI=¸R?¿‹æ0S¸l?¢f¸´¦‹&?êU
rìþé?¦Þþ'ÆQ/OTHER4FGL J1326.6-4729?×?««Y@-êy5v'À9C	A}À;å±^²<ÿ@Û¶ˆÜÌ@KÌå €©?´"=l@?àùíÌ÷"÷@'eØם
g@PôF¹?ïdC¬':׿ÔPá_ø¿Ô¦êk²¿äè+Íä¿î¯4¬¿ïÿÿ" 5•OTHERglc3FGL J1326.7-4727Omega Cen?aÉjKùØ?Zgg6RÉè?ïÚ4²öH,?j¼jíF‰?dJxð9ã?`³Äñì«â?ƒ—'ÝÿEä?ˆ`ÿU÷^?îkºõŽ?¦‡¼4i¸,?¤^oïHš?¥SÜÝýPí?fFŒ'T?Œ_ÇÀèJÔ?î ¤¹=p?›ï*=í֛?¥Â"¹•N?—'‰!HÇf?ˆ\›"ú?p&w¸œ1Û?íž"î"Í?–[DÊ4l?´@ÍJ[?•édE€A?až•—'nT?TgÞàÇgÊ?ïÙš›Ö?f'R("i?eUÐV÷?^ÜßGƒaF?~Ž˜G«®y?‡¢xÃé¬à?îi˜4"²)?­S?åj ?¥"©±ôí?ªÊÌäÂh?…
ÚÆk§?ƒ:©, N?î™ÒÊÜv?"šë"ß-?¡'æxϲ?'°©¡;³ç?aSåmø?L'œÊ?í¨þå+pû?•­rÕº¦?²/æ7,+?•sS¿‰PSR4FGL J1331.0+3032?ï¡5DZx@T+ü27‹À:ւè},|À<›µäRûP@ž&ÂaŽæ@ŸŒÝÉtS?Ç`ñ\y'´?ÅüÚ܄ü?ýšMÀg?ü´P^è×?æ)ÖÈÏK¿çñ¢ÚŠûq¿ç`Á`ÝæP¿ÚOó]ZN¿ì°-…C¡¿ïýM"ŽÇOTHERcss3FGL J1330.5+30233C 286?ïe·
Ýms?ƒÛ[	€Ò6?|v<£Æ'?oé!3ÜÇ[?ˆWù)?)‡éèïG?ï
°-ëÜÄ? ¬yɄ=É?‹Q+*vV?– ýëA›Æ?'d°¹Ü?ËÅÀÝä?ï,ž_Ï ?ˆ!Yq)p¹?{úŠc[p?xj)›õ‰?"ˆµ~y?">aH8a?ígôå?'W¼"Ÿ]?¯]žÓ«"`?ÂP—Ôä?žÑSEĨ?}yŒHLCÖ?îàý	£?'cĪ‹Ò?"GÈ¢â?ƒv…"ÅT?•;y} ®?‰3ôuɊí?íy"˜ AÌ?³{̋%¼?¡š²ä´Ä?§¿(»´AS?¦Ì®Â;G€?§=ºË˜o?îy£{Uòâ?"³Ö:`ƒ?‰Tg‡†n?"Ú7í¢ÈQ?¢Çp¾ðE?6懾8?çÙ+œÞ??­X©Ôïï?Æ$­/3Û`?­û³²Md?´íH¸€‡?•rZW½ÁAGN4FGL J1343.8-6208?Ú߂íП?»õ|"š7À8ƒ%{º‹'À:E×z¥¹@[#¨üŽ@ö"|#g
?ÆGX™Ÿ"ð?½|_LØ@-wœïo?î~՟ž?î|äù¿ÒŒewS¿æBaP™¿çÉâ!GÎK¿ê	ÿ\–¿åì†;OTHERsppSNR G308.8-00.1?¼Ì˜Î²Cù?Â,
ôy'ù?¤û@˜?Š+?«õ‡ Þ+?ë¸Ü³}N?Û³Qsª?©Ã¯(ãS@?°RØ«W{?·3ì¡ÁjË?°E˜n)?ë}Gyb#?µ¯ªê.D|?´‹Í_¤_? ìÞÖ½ü?Å{ˆ‹n?¯;YcÇÆ@?è¿
œi?±¨/=+½?"Ÿ #3|R?v~á´qÖl?¶Ø²½¿'?"îÉ¥9°²?ìì§]§{?–ZÄb>:X?°~-Ÿ£Þg?ÂH6§©I1?œõS‹€B?£Kmöð?í'aiÁ?´ÿw€%?˜j¬Qj?Ÿ°Ö¯Ì![?º_i¿X½?·]¢g™?ëüx½g:]?¸ ºÕfj?¯•ty'*›?š‹a\6BÏ?ÄÈøÞ3ã˜?°óS­eÏ?èÔj€Úäp?²o[Á6?wly×°¡5?bèõÞ"9ƒ?¹:Û±Á½?œ‹¤špÝw?ì©Ë•ëV?œâönžîOTHER4FGL J1344.9-6228?×P~Vêj¿ÏnëE2åÀ8¹ŸœÞÀ:4܃ùõ$@è8<ÝV@‰ÔDRÉ?Å¢ÁvŽö?Ý[ÔýrÜì@ìý
y@,:Z™Ô?ãH¶‡æ鯿ٕ˜ƒ$"¿ÚMy£¨¼¿èˆôe˜
M¿î¦âÂØWE¿ï×ÁÝÛgðOTHERspp3FGL J1345.1-6224SNR G308.8-00.1?}Ñ62¨ß?|ê[¶±˜Ä?Ñ@2$•`¥?È¢U"qi?ç%»K£ ?È¿gù'b‰?°ä($Š™?°;ߔ¥"ù?Ì\àð_ø?¹ïLdõ2?æÌB¿©^ð?ºãÿª€Ø¿?©ù$òSI?›Ì÷…5?Ûöϖ;ýB?·0'ÂÃg&?àeåêwz?µž¥J'n‰?ˆÎA7J?m¦\ؖ'*?ÁÏ9j-Ë?žÈP½çê{?ë(÷d>Ý¥? )ƒ¢…}7?†럍Þ×?²ƒÄ`MºÌ?ÔÆwBÛó?ŜkªAÕ?åDhÃ@›?Æbb†îi?'^WB>æ[?˜4^ßçå5?Ðj™‡·š?Ä(€~âÖq?ç7À½Ž° ?Ãû/Éú½ÿ?¡$KîþÁ`?'É
Áê?ß×É¡Zii?ºl­ŽEl?Þ¬àü¸+?¹ù'žªz'?iý@Í®'?WÑ萰»l?Ä?5P€\?ª'ôëÃÀ±?êÖ5š|Ô£?ªve2/MIXED4FGL J1345.3-6253?Ú›4ƨ"¿äâÙÿePgÀ9L[[piÀ:¼2JÕç@^WÏâ@ª*sq?Ïý‰˜š–?Úò²Ú³?]@!móùa€@óI€Òx]¿ïñ7æ Zé?ï•dSN\¿á`ÊžUì¿ç{wÀ*ýÛ¿ïÿÿÊPË?ïÿК·¦ËOTHERsppSNR G309.2-00.6?»<o`Ͻ\?À~­|qâé?Öy|šý"?ÍÖûµåÍ?á[å՘‰Š?ÍÚ¥Ž«"?ÓMÝÕÊ?ÈYª–A?¶U†}¡Û?°Ñ™§eÇö?ãŽmäè€?Ƃ<Õ7CR?Ì~"=DŒª?°å÷[Ì?ÆB§´(U?¬'Ž÷îÓL?ã\ÎFÁÒÀ?²ÌÍZö¢‡?ïáÐêê?©•ìô‡\?²"?ª1cÈ?•D \Æl?èÁµÒŠPü?®Ëbõ…¸?¹<EÕ/ˆ?Ãjõ]Jïú?ѼÝÔºŠ‰?Ê![Fo?ãúZӜ[?Í,9§0?ºOŽÉÉ?º†B¤À>I?ÀõŸ°gš?½b벖Õ?èx­¾ó#?ÂG1¤µ#?Âu[êXñ?©
äå'L–?ÆWÝõÇ q?­ô­ÄýS0?åÌÄ+
H?²sþÐwt?©Öþؙ§?˜tVÚ{b×?³ÀIr
Œ?¢‡]óIe?ëꖱݳ$?ªšnìòzOTHER4FGL J1355.2-6420e¿Ô(é°T¾kÀ•;›·À9¶N¼üuÀ;w™÷j·@%tÁ¾¢h?öªî «†?¼wbâù4	?§¥C_¿òã?êyÔ½\@UaµQ°ø¿ïòl~®[È¿ïì "ÚÅ´?é•\¾Fø?ïýaw]¿ÙÆ|¼A%¿À]GóÐGOTHERPWN3FGL J1356.6-6428HESS J1356-645?ÛÍGr­M?β"Ó(}ð?ghŽÍi•?Šˆî'ó¦ä?âó¸I0?ηÜK?Ýך_Ã?Ôøª1}?w4;¿öZ?‡«X(£?àægu…?Óõ§VƋ??ßçí®³uý?»º'C!ùá?¬ˆÏ?Ž€Æªlý9?ß
JY0E?»´rð8"?ærªÕ´°?¶ŒÌl—½R?vY£Õ?p"Žx™f?ÒÁF9}ئ?¶žh°·{)?ཛ*'#u?ÌZ!…G
l?"#6ïµïã?ŠÝPÇ{{¸?Ýã¯ô
9¦?̂r'n%r?ÖébÔ$sÂ?ÐÄOG2eû?uaTq"ò*?Žj[^7¨??ä`‹íڃ?кâ'¯E?×·:¼?½"HÒõ ?¡£Ý]qRÜ?œ2§Ô4«?ã
$ËÞ² ?½©7¾ª˜?݂øøú¨'?¾ èéõ
?"‰uhÜ4?šÁa
';m?à¢7Ú¯/û?Ã("AôuMIXED4FGL J1357.3+3730?•ü}ÉÂFÛ@R+µ^ñýßÀ;ÂD—Å¡À=ÅÉ£L¡@ k°'­¼ç?û'²z;/?ݲ~ñ"?ÔP`j£âÉ?ö‰ì˜D/?ú(¥é34á?åŊƒ| ã¿í]ï3ÿáÍ¿È`—D€¿áY+€Á¿Ôãr@9V
¿ïþëbº	|OTHERgalNGC 5380?ï²ùÿ:?uÆ)ù°Q?]fŸûDx?VÏxWckñ?žÚõO:	?r	ˆ§?ïAÔ¼+·?—^Ÿ©›H?xjvÒ(†#?ƒ!]ӱ̣?'ªßYolj?'L-˜#(Í?îúSÛ@ÐL?'$(³(?wÐçé\ë?{éáƇ 	?šÁJÔÖB?ëa¥pï*?îz$œ á?… æXÔ?|Cúí¥Â?gh)µ]%ê?¤Õ6Ԃ—­?ƒ.íÛQ?ïT›¦lÄW?ˆ×‰žŒ¹?m`1`N?bÂù¨º¬3?'É™€]ø?†|eÝþ™?îh:
dcú?¨åYIEº?…‰£kû1×? Ju4¯?¤öMßê?¥-2˜L >?îe'ÑD¤?•çUQO¯¿?|ªeh´§?~C©$?¦@}Cƒ«?"Êf[¢¿½?떫$}Û?£ï}eE?"	97ú°D?€ó¼ì(3…?Àd¿Û€Lt?¢™À> ®õAGN4FGL J1358.2-6210¿í¾ùKA--¿ÓwÂäì~CÀ8SÒkr>âÀ:WoÈ@ã'4pJ@[#<E*¬?»5€•f¯?Ѭ‰á?Ër@íwàmò?û'ºz9×è?êœâß]É	¿ÛÖqüœž1¿ãŸÕÞCl¼¿è±·Ÿ¿ì踻Ð`¿ïýáÃÔ×OTHERsppSNR G310.6-00.3?"ZŠ5üÑ?ìóaJÃ?¾š$]FEù?³ã~VQƒF?ë‰ëhe¼j?´'˜û?£³—Äó³˜?¥s£Ñ<.?Çè´mõÙ?¶ +R­æœ?èʙh
D@?¸GDú¤Ú?¸?Èعy?¤ãcݸ?ÑÔ¯DP¼Ü?°\ò¬"ÏÚ?ä
¯BÎ0Ð?²oR Æ:‹?"n­Z]Bø?i9S/'?Á5q'gÆä?8RÏ'<|?ë`èæ2úS?ž¼Áù¢'?…³"t
†?y;OónˆZ?ÑR¬Â¦?»!^t"?ç&ˆ[ó_¢?ÂÖ°8ËM?Šƒãüs–k?-åzõgì?È6JÿÓ?¾%Å:Ã\?éˆI2ôR?¾¥¦BI|?¬ß|äÃh¿?š9h_›0?Õ|";(—?·¼¶!ú ¤?ãs¾"¤9?·ýWsj½?cÚà@‡¨?Pž®¦!	‹?ÅM¶À¾?©óA? ?ê˜ß/% ?©9o¡VOTHER4FGL J1404.4-6159¿í·jŒ)³G¿Ôq1Ûð+LÀ8!‹P*º¿À9µ+†–‡–@–#BzN@í§m—³?Ä9å>ˆ¦Ø?Ø+G¬fû¸@…ÂL@J?ÿBe"C¡À¿à-Ný¿?¸óºLl•*¿åA1ÃÇj¿ì4œŠâ¿ï«±äéú¿ïäa¾áҘOTHERsppSNR G311.5-00.3?´;yÀx?¸X^gž³?ÂWÇÎF…²?ÃÛò‹˜f?èâ­Ê±$?Ǿ¶B¶w»? ³ÝŒ"v»? Èªmñ,û?ѓ@â§?½p_Šù?æ+<†îò?¼ÔV°™n?º´	ôJ•?© ûðs=?É
\Òé?±À:z÷®?æf'™Ìð3?²ÅŠú¦>?u0?ÚÖ»¼?]-¶j?ÂVU0Lè«?ŸW"¢¥*?ë@
4iò–?ŸäSqÚr?£}¿û"?¿Q¾+ÒÊE?Í?Ñr›J?ÇyZÕ
¸û?çxnzYt?ÊÕèÕH$?Œ`'T} ?šgyš?ÒÚ>åE?Ä~ø*W?æ!uw?Ä?üÏôÊm?±KI'`¹U?¢ä/—Ã7?É7àü­Õ?´hy#	¨?爞̫· ?¶	¤>P4?S.­ñJ§?B0)¨è?È'´Ølñ£?¬Vïi?éì{s
[?¬däsA(OTHER4FGL J1406.6-6523¿íúŸpž"ÀÀ
IJFu/WÀ:;Öç‡À;‰5
þÆD@؆V›Ã@,ò;ò–?Ǿw‰ú?L? ƒy`'æi?܉±¤Ó3™@7~'«cœ¿ë; !³ƒû?̤ç«ud0¿é"kaøÃv¿ä¬åÁX¨¿á§@¡/å÷¿ç~Ò£¦bÖOTHERunk1RXS J140629.8-652251?à•Áq¹V?Å),õŠ?l¯y•nA÷?`îR{žl?ޛý¤¹'?Å<ŸÐaÏ?杜U?ÀK ~>Ž?x{ ¹‰H?#ûjŸ¸?Ó{ÖCÝ¿'?¿´òÈVgã?ä¬ÿŸÝÖ_?±ê*ܾ?–˜ý@8?ˆÑ·X¡u¿?Õ<pç§L=?±lƒ¼¯z?êSÝ4†6?˜:ܾÀF?oïé¿Ç5?cà.ÍéÇ?řŒ1ëÏ5?—†ß½R7?ÓÏ õŒN?Ç7/IÍ?}æà퓳P?t‹\Ås×.?åÜaÃr
Â?ði\ú?Ù1âÂ)u?ÅáÔ{Ë[?|\¡6$?‰À}€ß?ã.Vø_LÂ?Å®Uþº/¼?Ø î×'ˆt?³!ö=í?£L$BjãÃ?Ôß÷¿A?âzÆP"Ê?²æQÓ{Jv?â¨zÝì¯Á?©Ù:l®?"¢oÚm??Oª<Êû­?ÙtãF¶È©?¨uÝ¡¸aMIXED4FGL J1420.3-6046e?ꝁºÍd?ÎÆŠÖ8À8ÄëVûÀ9CQÀ¼ô@$ýýÇ@œ?ÿºjyñ]¦?x´u4ß5¿Ž€ÚZÿÕä?áÉD6¶Ë@
1iEhêпÁ<õ(áu¦?ÏëIúõÕ¿æž¾°nÈ¿åæŒÇ#? ¿éQ%Â1hX¿¦ÀPë!OTHERPWN3FGL J1420.0-6048HESS J1420-607?˜«(¶x9²?¤7Ö+×Z?bÊèò¡`v?pÿH2{U?ï'ÛÑ*?¥&ì-.D3?¹I/¼âó?Â_	Œ?™Ã6hJUß?¥ُïDô?ìĪ"?°‰Aª?э®ãÇ~ô?²®í*õ©?³¾Ï×?ظ?¤óâÖ¶?äÁN'ÆQð?²³Ÿ}a?—4e)¨Úz?…K"EœÙ?sKr™zb?gÜùÉe}?ïÅñD?‡Ç-Œ¼L³?¥tKú{òð?¦é¬Úӛ?dð†/'?p8ìGs×r?P
+?¦ó¾Åvaô?²Šÿ"Øç?¹	¬¸®}n?›Öë<W'?±ÇEê¾üà?ìÖ>hÎÿ
?¿U߅Œ'?Ö·Üö:¯S?²Êd!Š?¯¹³vÀ?¢™¤Øò1ý?â³Å靁Ê?²Ðr$³ß-?{âz>ЗR?r±‰?N]}?~'"¦–Í?[(§?ï‹äUÞ?ƒ´þÑ4.OTHER4FGL J1423.3-5655?Ý:FÝ"/@
Þ軶$À9ËýíאÀ;€Px@Â.jÑ@´€Ǒ?Ô((}¢˜?á°:Zná_@	3ä%®æ2@9q‡VËê?ï¯oYT/,¿ÞÀ£ô'b¿ê_$º|¿îÚ®/ªè¿ïâô˜VN?ÒÐXþý—OTHERsppSNR G315.1+02.7?ëà¬søœ?¹Õ²l¬Ú?¡85Iº"w? ˜kHÝÆC?¸^¹ª»h?µþK;eýM?á½ïº7Ÿ?ÆæaÀÂÜ?»©·Iü"?²§tD¯ä?×NK¡?ÃíÅ<W?ãè©-¨8?³mô2~?½ja¡Ž8?¦hQ'M›?ÐÔ,
`L?°h´Ñ™ÀO?Ø¢\©×²â?¨¯×'=A?ȪŽâUd?¡³J"ªš¾?Û\O·"l?§è"Yµ?æL¥í\[Ã?Ć4ç,8\?¾9x Q?¹>ñ¶[ß3?Ç°¬:†
Ì?Á]QB_?ËÕw­Øã(?Åփ;֒@?ÑAÈì -?ÈÃ>LZ»?àj¯ŠFÀ?ÊeWÌE?ÚwuÖ#–;?µb¯æv¼×?ÈGm¬½°?±+Ñrà?ÙdÓSϊí?µëOFs³ª?¹ÐÜ*Q§?šäRŒ:?ÓwÍ?þ£?³4r
T?ã	ýÚ¶ÅN?²¯²¸¡&MIXED4FGL J1433.5-5457¿ïÿ÷Å¶@ @¿ã°>À9â2²Ú³?À;šÙ¯3^Ò@)áҏi@5%£þwj?Æ©›o\¯?Ög^~:˜'@Pu-©†w?úX×d«PP?ÀÆtÙpÊ¿ÊýpÄ
`'¿çÇ}³^g¿åWl˜¯ŽÎ¿ëi…ÀçÇ¿ïúñ"l'yOTHERunk1RXS J143329.9-545931?»‹ºL±?°Õ%pX×?Áü#Ú±š?³Õ³°

?èVʒ
?¼˜àûÇ¥à?п%¯¼ñ?¾³C=3+?ÐAºVõÒ?¼ÿJ<SQ?ß8˜•ì ?½½ÐÒã3¹?ؾ6A?²Bèåò?ÄbÄêÄô*?©š´µ?Ý›gDæ?³)%îE%K?Ó*Qdn? {¥4VÅ?ÒznõÅÙ?¢iÖÓùÌ;?Ú¾4,œ/?¢cÈìh?¶[Áf¥?«sJÚ¬¤Ý?ÃU"Ψ¼o?µ""ª«	?è_&Ÿ¸'à?»øÄ{´E0?µ"Íˆ¡‰?°¬mƒQˆÓ?×úø½ãÈ?Å©#²Y&?áPf	ý¸[?Ä+=Š=õÉ?Í-{Ž@Ë?ª",T26}?Ç֑5‹ÁÙ?®{e¿áý˜?âȐTBï¶?³í0É»9@?·—ó·ìA¼?'?æs1½ø?Ù&×@]?¬Qµ¦ÖÉ?àŠîTyª?ªšØíOTHER4FGL J1435.8-6018?ÊÚrvX搿"`Câ'íÀ8†µò•´2À:'s‡Ù~@Wꞙގ@Vžh5s?ÇrªÂ`ã?å.J€¬¸°@÷jrd¡j?þ%J~¬-?êYà[DŸ?˂&¶M.‡¿åŽÓ朂¿ïQ¢£Y6¿ã3*š}£¿ïëÊSuÈÚOTHERsppSNR G315.4-00.3?½	nØi§Ó?¹'&‡µ?Κû·y‡?ÊnTYÒ?ä¸7iD?ˎw‹–j?¼×åÅJ?ÂÜÕ' à?Öu[U¤³?ɑe‰'ÜO?á*U;ÔÂ?Ƙ1M£@?¿¨¡88E?©¯ÚNš¶³?Ê8‰ùwé?¯N"o¹?åŽ(n"\?±à|~—ï?"Êmÿ?i8ñ¶ïö?Ò»GÃEe?°;¿³Y•?æO4C‡ñ?°#¾³øn?¦"ÐD(?£ïšzf¹Î?ÉÒ÷ž²ˆ(?ŪkŸœy.?è!õ-xM?Æåx¦ko?š÷,ô_ç?ªM{ÉOä?Úm݇~Ü?Ì@=»UÏ?áñX§?ÊÎîDþQ?¸Ä¿C>?¥?¤QJÎÅ?ɓ)UíP?±±LË"è?扂ÝëX(?³ÄL8§a9?`›œIëe"?LùŒh[?× ¤_ñ,S?¼–û•É;¯?ä_45Ù?¼"˜g"7vOTHER4FGL J1441.6-5951c¿âà7Ú{¥Ø?»AV¥O°À9¯ñŸ,ÞÀ;Ld\ ë@î«8}tö@üÂ]Þ?Ñ+L§?ïþ"ƒÕâö@Ù"d¦@Ö m³·¨?ê®=Ë<©Ô¿í'úðÍ¿w%¡'ϱ6¿áY¥-Ã¿ïüwêó(¿ïàzßDH¯OTHERspp3FGL J1441.5-5955cSNR G316.3-00.00?³¬ûàCs´?³ÐFM†	‰?Õe$îFM?ˇŠ
ãçN?â×Îv×3?̎¸È'‡Z? ¹Hp
,"?ª8åöO¹7?Ôiò{ÌÃ×?É"À¡g»?ä¿r:ýNl?È=ý!åi7?Ò'Üéá–Å?±)mä>k?Ó¾Ym•ÀØ?²Ü窧;¡?Úɨˆ¨c?´i¬NχA?´èȁK•?™'¿p?n…?ã^½µ$1?¸¬k"­äƒ?ÔR'iÁ²?¶Â′ê? E?è1Þô?¤gFóõÔ°?Ú¨KÊ??ÍÂˉÝÔ?á÷×ܶ	?ÍäŇí0?ŒxDÒÙ0?'Ψ/Ž¬ä?Ò6
Í}:­?Èí÷C1ǽ?æsKÛ ¥?ÈàQ=™$?ÆwCêv½?«å]ê?×h¨àßS?¶àe'ò^Á?Ýî[¶<Æ
?·"€e	&í?âA<Ü
u?ƒÃ÷u?æ}®þ/?½@uÑhgó?ҏù)Î?¼lâi÷ëMIXED4FGL J1442.2-6005¿â5M8m¿Á4¾x¡&À8pM'iÒ,À:'_lw! @¡…èÜÎ@Èú½ ßß?½Vx¡k8ø?ÒCf;ô!û@‡ÑÜ×@"Üî^B¿ï§vÑîu?靖¿µ¢¿ã'8Â>Sx¿å"°üŒ®¿ìÒÔMʎ.¿çÐV#ùŒOTHERspp2FGL J1441.6-5956SNR G316.3-00.0?¶ØÝþØ †?±F>ڄ'?Íñ(]?ÉÊñúÈwl?娝xÔۘ?ɨÄs¦¯›?¶‹d¦Š??´û:P6bã?Çm–Šæ?ºõ=ÙÄ?çi¸s?¾W$mâJ|?ƺB}öGg?¯"k¶¡+"?Ñ­ê1?F?²z-	 Û°?ázçëó>ã?´Í훧Ðd?³½UÔéhô?"lšª]-¥?¹UŽ=¸Ö?–ÜùM…Û&?ê]£}âȦ? ÜcÞ?ɖ?¦¦‰ì‹Ö?œ\¶!U3?ÕbgÖJq`?ÄFûS'D?ãäc"‰½?Ä_3ÄJÂ?¥çí?±Ò;¸Èý?ϜZ!1?Æ{üZð?æÈÁv¥?ÆôŠ+¦œ?ÀÌQx~Ó?§'V	g?Ôw'fÙ]?¶ƒ5M@…?á'WîÔ^'?·£IÁv?˜Ö…PUf?ƒC.ì85C?À"g?§VÇPÐÁ¾?ëeê·æ®?©˜#zhðOTHER4FGL J1443.0-6227e?Ò0,ù7ºÀ.>ìÀ9})ž^û8À;ŽÿӊV0@$+Ö²ÿœ-?÷ƒM&ú@?¸Õp_c'Ì?»"™T¥HÏ@X¥H#…@@O~JˆºN¿ïü@ø¨ž¿äpaǛ4¤?ïû
˜	v¡?àÑsZj¯¡¿Ê[Ym¿ÆÞ°zՂOTHERSNRRCW 86?çÇ?n¢A€?ÄÿÐ;¡?WóÉíõ"w?Peb‡Ã$?ÐYY3;Û?Äû'ñü ?对ݗ?ÐiëÖ?l.0o×z?€F.¿Ygg?Ôiª/¶Hs?Ϥ(tÆÚ?æÑ[PCö`?´WóÆÐx?ˆŸGÅ?‡$ܱ°âm?ќa"b^"?´_ÓáOL?êo˜y^Ö?¨ÏD¢²¢?r©YúÎ

?dÔ¨©:w?ŬSK'¶¸?¨ëfÖMÔõ?ãI×Ô+«?ÆïdÐáÌ?sÍ.SõÕ?p
š(Xæ?هdBR?Æë"ßÝÔ?àƒñÄCð?Ð.GÉö·5?tŒZ2"×c?Š‹œà*?Þ¥ìY–/"?Ïÿ9ËA¡$?âr­Mƒ?¶5#@ís?#ßЂv?•C/FÄ©?ÙHfÈÙD¢?µ·7jHŸá?äÏví•?»1äWæy?‹ø:+"'?6=y"3?Ö$ðŸå¹?»»`å4ùAGN4FGL J1449.4-6026¿î|Š(§,ï¿ê]îBhZ\À8ÛM²:zOÀ:dåÏ@"'^±Ž@ºZƒÚ?ӛÍÐeß?ÐÆ÷ µí@ºç"Þ÷r?û…K'Mð¤¿ïÛíÒ?î@œ<âž¿è÷ŸsÎ-ö¿ê^áÂ}=˜¿ìÕl
?ÆhڟsMUOTHERunk1RXS J145023.3-602718?àðëÞh‰4?ÑCƒÅ>Z{?½ÝÍ ëÄ?Àl;—?Ö¦´úóü'?ÒrÃ™êš?Ƌ!¾Ž?ÀØȽX‡?·â¨A?Iô?«P#†|bO?ç`âˆBPª?ÀíaöGÍþ?Í)‹GO?¯§F#¨?«{õªø£?«(Œ)-E¿?ä›ø2p?²>E» p?¾D'6С™?š|S¿n
7?»—5óú/©?šèÛ°œ=Ù?èĔZ¦¥Ø?£"¯¹?Ú©ãÌtý?Ð)"TK?Å ¼-mKˆ?Ã'2ƒF,?څ¾×|å??ÓýÉeJmÉ?¯a¡*"™©?­"†9}j³?¾iÿ֘?ºêš#hv?êI8­'í$?¾JMMˆ?ù"š§?§Ëª°9»…?Ä"ÒPLý?¬×m)m…?æ2Ý,š?²ãb{b[q?¡´Yú¢g?‰š¸0;:?¼–ôƃ$?¨($J,áð?ëQÛÇ]ïl?©:i¨MIXED4FGL J1453.4-5858¿æPÁHµ%'?ÐÏ)~(¤åÀ8ö—¤ÌӃÀ:Z‰%®r@åÀb[>ë@"&~ïÊ?Ëç€Ø,§S?¸MŠÞ|ô?ðx×ÒºL˜@ZÌ´ùòJ¿ÙèyÑ}5¶?ÑUÈôÐ÷Õ¿ç¦G'Jˆ¿èʑž£n°¿ê €¾Z‰¿Ëºzå¤_OTHERsppSNR G318.2+00.1?¾.?)FÜo?°[":w"¶?"é›Áe[<?§çϕP ?ëšë<¾;(?´®JGû*ÿ?Ã=ޟ"?Ãd,ü?œSÉÑ{Ð?¢òÁêJÖ?êP¹¨WÍ?Ã5"Óº…U?DzӞÅtá?¨ÄðîՕ?´ÉþÒR?¡Bג~?çzF&¢N?®FË+èD?ÐÒ{?¨‰*q¤d?•&ÖrVÎ]?r†+;	Ç?æíÁÄ'" ?¨º"ë"çû?ª€w¯pÜ?éÙðC@ê?€Z`	á?|ÈåY²0?îç»æ? Ì0‡ä?¸'?Ònp?´åº*D}? {V*?§ÚGº¢Õb?ëìWGIP?¶ò,¶?½°ec4¢?£¢Æ<Z'V?³~¡´å? ¥·3XS?éÚ2?a{?©´ÀZ†Zä?¹·cÍ–D?ŸÛ†C¾€5?˜á±$>'|?)lûHèª?ìü÷Àt? «1r¥OTHER4FGL J1459.0+7140¿ïú?iLtÎ@E
c
'SÀ:*ŒžßS¸À<¿45'²E@"w¡ÍÏ@œSE!rA?´Æ¨à"Xß?²)"ø‹?ö³#ä
Öô@mÆáü3î?ÞKs0yD¿áÁ~_¬bõ¿æ|yÞ=bŒ¿èL÷à 灿ê¯þàÆ(ï¿Ù‡÷%ÛOTHERcss3C 309.1?ïô´'9Ó?YíC>rô?>"GŽ*¡?@OH¶@Gu?MíW4Xòì?R¸2`ûB?ïë~Âcù`?g³×ÑR6?5*EÕ {£?EÉú€ó?aÛô܃®?c´åáéð?ï±@W$'?{wnÍnW~?bkA(֙B?q·Ñ¶.²?~*3ޓn"?u1åÓk?ïü¿¦n?Õ%ú¿€x?"¨›tTãQ?§#'ÂÕp?0®ƒT¨g?4Ú»cuÕ?ïð^¦Ù?R¾úBl?Fþ渀¡B?>r|ëúaî?SÃ@Mú<"?P('i†¥á?ïÂXçÅ?€Ž
Uז?Fo®êÅ]?VK1«˜zƒ?|–MLú†?}AÆü­ªé?ïváÄç·?ƒŠ
#Õ%A?oÆ+]§×?wò÷«^V?ˆ0¼´œll?~?={K?ïö'ÐEÈ?B†prI[?;©s	³¨?)°ÁY?IŒêfD2?>ïˆléÓvAGN4FGL J1459.0-5819?ÆdàÝÙm?߇ø\rœ«À:Qo'TÀ;ü;ëh™@ÄŽ˜‰¤@9&Ÿ¦ùÔ?Öÿyvƒ??ïÛ>w‰ú@
q#ˆY@,©óXý?î@Ôqü™¿ïÿÏX˜GŠ?ïýP 슿äÉ>$'ý¿ïÿü¿ÙŸC?ïÿ•!îZOTHERunkSNR G318.9+00.4	?ÁM×0Jm?¾¡Pа?Ϫmøg?ÊÊ_KâN?ãç_'æ¥?Î~4ZÇï?È׆Ç?ʤ-·š$?Å ¾(;ªÈ?ĸ09ÿ?äaîÒ±\?Í{ˆÌí®ð?ᗳÜMì?±ñ‹áÕc?ƁE¡/?«§o1ו?яØ=vá'?°òCûe?ßv"ÒÉLK?·…Ö:¬?Έb½º?·Þ,ÛÞÁ?ш·"…TØ?´«!¢9¶?±­P\n'ì?°5̐1©?Ó2S`
'ç?ÊÕ×eN†?ä1,Dzï?Ìë1ÅRŸ?¼ÖéÏD©Ü?ƄoˆE€µ?Æ1]
TÚÖ?ÊU¯Jþ?æØ˂Â4?Ï"½&3ó?Ö½;ö·h?³v¥2Zï[?Ғ$¿íÊ?·[×ó^?Ö°Ÿñˆª?³ÀòÁŠ?È{Ÿ!‡¨ð?³õ¸@ö*Ä?ÖÌ,LþÐ?Ådˆþ@ã?Üö!*z°?Ã~ú,½‰tMIXED4FGL J1501.2-6624?Ó䏃ÛÀ÷ /µÐ1À:Óúœé°2À</†K<@F6­;7@³©ìiJ?ʈüˆý?²¬¿¼°?ì‰8ž2Z?ÿ<¾U¼u?çåWr­œ†?é:ÂG¸¦¿é6Ä¢–¿åË·Ä'Þ¿R'4wU÷Ù¿ïü« —OTHERunk1RXS J150054.2-662400?ìÍ]¼|P;?­GªWM?v»Ù¼Ÿ°?ƒ":p§zˆ?¸)T~…·¨?¬,âNÄR?è®dlï ?À­¯§o?qdˆuÆßÛ?{N§²Pê'?Ì»JNí"?ÀZEӖ7?í0xû‹Éo?É).k†?"æ×I"V²?`¥
–m¢?³ß];M³?›5Pl`?î™ú¥Öœb?ƒ–æƒË?q9¸3ëÆ^?`jR´£ÐE?¤9žj}'?'‰{äC?çðÈWЪ?¿4âgz?‹Íòv0‡'?'6f{á­?ÎÿzÛ#¹?¾©e²"ðÆ?á³Áù_'?Æ EEÑ?u=õ`ï?'R$ruL?ÜDeÍ0Â7?Æt~La,–?èýÃî½ô~?¬2r¥Ü?~?•ºæÍ'[Q?‰#œ×Œ?ÉQ"l?)?ªÃæG'Ó¼?ëîëµñ(?¡Ÿ³Éw?‡ᄰL?m$[­
?½¤¦v.? º†Ñ¥UŽAGN4FGL J1503.6-4146?ß)ºâG;@->X¡UPÀ:ôx'Y
]À<_JÚåª@ <','Û@éLz,	?ÉVöœT	?'Ÿk¯j?É,{Éz?ýH=ägF?$_öŠ¶¿èfÊo${
¿rÈÕ`3
]¿çÛêw¿¿àŽn—€¿à`Ý?á—_OTHERspp1FGL J1501.6-4204SNR G327.6+14.6?ï9÷‡'ã?}…¯y‡?Q"ÚßÕS1?@Ø$ÂkèÜ?—§Ñb*9?D¦µ0?îÁ E½õ?¤Ë!ãni?vä›Ä@à?x>Ù,øÃ?¡h+d<(?£OÎÞµÔ?ïU
Ö?3¿?ت™x¹ß?hhOK¾?gH—fÃe?'Q›QuU§?}>`Rn†?î3e0S?'àΣ?vJx‰%›'?`ùÙ»Í?ª 6¤~e?é\r@=?íý€!+&?§€e"ØÜ?aC]R¹†Ú?Rìº fù?¯ò('Æ«?§ZŞZH¡?íei`ì©â?´~Vê:?ƒkÊþ'Sì?Ž4K_o"G?²g;šj6ñ?³v©îjE?ÀK×f?'Ø)ÂM?sª‡
|?j;5ºlc?¤ £'ˆç?¶Ó<þ%?êø§XôãÂ?ŸêÆ­¯îH?‡Ú'2d?zï!î·¸$?ŸÂ[7fÒ?Ÿß\ÖÌ~AGN4FGL J1508.9-4110¿ä´ MÓG@-F§&J¥À:ÝÿTßUfÀ<'…o@*@Kڔáy@ñã݊Š?Ò'™¢ÓÕ?è~è]¡ñ­@¶,ºs-õ@y,¼¡†?ï)'Dé>¿ÒփDm˜4¿à(֞椿í'Í+d2¿ïÿß^IâL?¼ð&n(҇OTHERsppSNR G330.0+15.0?× 	0'~?Æp¢›\"§?۔ä,A8?lj¦m£­«?ÊÎöñl?ÈÊíµ¶ÁÚ?àšaïD'!?Î @ãÜ,?טI35ó"?˧൞@?¼Ë˹ ª?µ!‡ñZß?àS4G&Òt?³ùŸü¿ý?ÔÒÐÓ¨ÅB?°‰,Fiw¼?Å
<+¬?©‰eôðe?ßupp'žµ?§ C	–1?×ò'×çÍ?§zW*¦u4?Á/ùo¢ý?paRZ‰Ç?Í7M{Ëå?À"…7"H?Ýø#ï¿Ž?Ç­^•âÖ?Ól5Ž¾Z?ɶ Kº?ÌÁ"Ö£?Ê£É;{^Ï?äa'Oê½½?Îú§
þùÎ?Â\5,h?¼Hîmd?Ô<´—²õÇ?³¬W÷_^?ßR }ÛÅ[?¶ÎÒã÷'œ?ÈáUÔ≼?¬û~qÀÑ?Æ®€0'î?¤Y¸ÇËõÑ?âñg¸Îé?³£V¹x›Ã?Î4µ(ì2n?°P[ÄC=MIXED4FGL J1514.2-5909e?ïÙāq&*¿óW"ëïyÀ7§È‡Ã®@À:ä¥Xê|á@!Á»¤[iˆ?ý<96's? ›ªãÔ?s©…ž/Ãw?яãÉén@KûXÑRn¿æVc"3Öǿ䭕X¥´¿åÌeÔp/=¿ÔuÜyh¿ßÍ܁˜¡¿É(èÁõÙ6OTHERPWN3FGL J1514.0-5915eMSH 15-52?Þæ'pþ?ǜ³®²tK?víAŽwù?k˜jòs™»?à_sûœ»?NJ!à<N?Ø(×ÚÇâ,?ÐýLÜÒ~h?–úBŸäk¸?¢ƒ=±Ÿ?ã3Áýª©ü?ÐôººÚ²?Ôì›ëi¬'?µ+'¢¢¥ß?¥¸!2E?™ÌRêÿ*?ä.0è*KX?µ}O½Ö°h?äÇ®ò¾›S?³,\5}=Ø?©jðÝÏÞ¸?"}¨"ì?ÓCCþÿÇB?²毋™2?ÛTîäçå?Ä[ŠA"Q*?ƒN©Izž]?vûdbɯ|?âNN}͜?ÄQtðJˆî?ÐöÒp`÷M?Ë«çœST³?›³!÷Ä?«lâN»»2?æ¦þ¾Ù¼l?˦áQzWE?̹\5>?±o¾À•h?¡:#<p?"´úÊÁAÅ?çéä¯0s?±í†®¬ç"?Ûiq[¬?½T–èÚ­?·™ul~â?¨û"Êý³­?Þ°–N;û?¼­¤Üvk MIXED4FGL J1518.8+0203¿ç‰ Ýñr@G]{á!îÀ:¯c>"¹†À<bã¹x\2@NóÄÞ@è@,¢Ûa»?Ð2&ìS?Ýï!‹k@Û·-[@9È"Ãú@¿ïÿýF\I?ïÿíUÙPi¿à%>þÃj¿çÑt!N¿ëçÇ$_¾¿ïRþª•jOTHERglcNGC 5904?íÚµöÍ?§=qûoø?¢°nŽ§Bè?¡Dz݅›z?ŸHˆ'؇?•g±…˜?í6`妖
?®íßDˆ@?¨¡Øú?¦k€|s5Z?£øïŠNék?—wu
 ÈÖ?ëÍ*ö×?ö?§ŸÐ§c5ù?©ü‰•úÚ{?œ/×ó—Gø?´˜c'm'?¢Œ@¡£à?éÜ¡ö¬¼ƒ?˜e‡Ä/s?¼VKþ!??"á&`'™?´Ä¥?wá¤?Œ?,΅­«?êæõÂåB?¸ ÊÓ§0?½iµ®Ö ?³ï þ‹q?±^œ9ÿM?¦å=I›b?èé·&%?Á»"¤ßa¿?¾Üá`
_]?¹"D¼V†?¹Ú¸æÄxH?±Gƒ–?éKü$J¯s?¬ÆØ6Ð[)?´¾ø*¡þ¾?¡¸¿d.}Â?Àp"YOU?¦½4iÄ2Ø?ãžWë"%P?ªîbí·³H?ÊK	~.I?«ëƒLj?Ç;–Ó…gw?¤ŠÍ×lk—AGN4FGL J1528.4-6729¿ïúéâÿŒÀ"X%[À:·ä‡ÔuÀ<qfŠx"f@!
Œ!¶Þú?ü¢î¬ñe3?ÈZKæ]l˜?¿ä†Ò… ?ú0– ÀÕH?ö¿Ê"xzæ?ïþŽø›ˆ¿ÝLr^í T¿ãÜT)M¿Ñ¹Á¢w8ǿݬðäY0s¿á$I@:ؙOTHERunk1RXS J152815.0-673003?ìQ§®ôä]?±‹,_Ø£]?Y§&o2l?XhîV	v÷?½Wí¸æÍ?±[dq(?ä±·
%‹?Å8ÚUæ?†qfmmß?V¯ñ(0?Õ鵌ûb?ĸ:!Ü?퇜%(ó-?œôª¾-m?v@®¡®?rœvéy§?²_ê¹3ø?›TÊmÞ'?êžnÃqë?š{Œä
ž?™ÏœÀ'"f?|Ì®cãÒ?ÂLT7 d?™'Q'Ȉ?éœ H?º b'x?eŸ–@ó2?`ÁøGiÁ?ˏƒ7¤ÔX?ºãE<Ó¤?×ϙGýù?ÅÜ&©Yw?ŽOT"t–?•öRۃħ?ãžö!˲?ůè¹E0?êù+?«§ªÿGž?'|‡ï.íÅ?wÖÓ7RX9?Ƈ㝸{÷?ªÉã5àZË?âÖOÖ¾#x?¬=´,Í%~?«'Sçúë?–K7
ùÆ?ÖáÕ»o?­Å…•1©;MIXED4FGL J1533.9-5712e¿ïÿYõ׿ïÿ"ÞïÀ:°ßé	CvÀ;s­íät‰@(ŽÂ¦]¨?òUav<??ÕÂZµX<?´–ÜO÷?â	>m#
?ô´ù[öö¿ïÜb¦-¿ílÚ>$}ä?픁+äŠY?ï÷ÂCÜΣ¿ä*X-¾,?Æ%{º‹©OTHERSNRHESS J1534-571?·þ¨/ª)Ä?Ã0Ü.1l?ECÝ»¤Ø?kwÔ(¸?ìúÚ9g?Ã8±ü«?½ŠåÈWƒ[?ÆÄZH²?"΂À TÛ? Ç؋
ÏV?ë°/14Å?Æ5ä'9ðV?Ù€XïŸ$?µ…"!?ô??˜7¶î³	?"F߄׸?ⲇ½µ=ö?¶fƒ"¿
?ºPïNàkn?«G
Œ"$?z•-ŒÊ»?xþµ«‡¨Œ?쀷»B¶´?¬3†Êqï*?ÁtNCãbC?dž;'lš?`	F+¨b?|ÂÉùÉ?ë'ã(ü?ÇÎWD19?¹ÖaHå«?ÃN=Z~{±?"ò=‰HJ?¥
 ½ÕW?ì,tKÆè?ý,þˆ(%?ÕÎûÙ³C?´Z‡o5ó?§Š"'rá? r~ÃB?ãùp?"PÁ?µaO	ÚGª?œ˜É'"?"Õ>öÛ ?'\è•Ø}[?•Ôèb"?îÑÆoö*?žâ'D'0OTHER4FGL J1534.7+2331?à¬uG"@J‰,à2ÛÀ:rÚ:s™UÀ<t¥µ0Ï@£àE$¢L@YÚakU?¾/$…ÆS¿ƒ@f«
gû?ÁÃì¾Ú›Â@y͸/0ð?™t6!"èD¿åaþÝÁ׿ä]`='l¿æ·a*½Bì¿èÀ0§g¸v¿³XƒàÛޟOTHERsbgArp 220?ïЩvd?qHÇ6cS?\‹7¤Ü–¸?RªÕƒ61?pˆvß?ù
?oJJòܜÊ?ïßÖºŽ?o5ñÄüî?AáI˨‹?M6z(?l†éÐ&;?iæ{c¿hC?隷ÿ"A?tŽ•‡'Û?a{Ê<ØÛ?jՐ…aê?u
Ÿ+#!?i›MX\¸?ïÐògLP¢?RŠ;˜µ€™?Z§±»?>?q«Ö¹?q‡×í²?LÔHê?ïŒç‡Á³r?'"&
þ¹?v‡rÙq
?t߯¬½l?ÁÚc4îú?vó³E±ë?ïAý%… ?…Ë'þÕ?Q÷iY€w?]ᤄ^?†p"žªeõ?ƒÖçðÏt?ïböŸ%—?€ÙÌL翸?kTs™…š°?o ­¯Y)&?6®£­I?{˜kcÖµ?ïw{‡4è?pnnÝØ2?r"­ªÄÎt?YÜ ¨ú.3?ˆÞÇPUÎ?kBk.RûAGN4FGL J1544.5-1126¿ØÙ'ê7@@9&A³À9=ì0?bìÀ;ÈRÆvq@âd¬'ä@5†S€?µaL̆Ç?ͽyȘá@ºx)‰‡?ú¡®÷Š?ïÞðáT[¿Úiþ Õ®¿å®í¾´Ü¿êy…'ͼ¿êlH"ș¿ïɞs`JOTHERlmb3FGL J1544.6-11251RXS J154439.4-112820?äøû'±BÙ?À=«-¿´?Éÿ1Ÿ›w{?½­ä`	?ÂàÅ>Ÿ?±Õö":¿?ÏîÅ1ÅA`?ƕk2d<|?åˆWœ
2?ǀ¢ÔÎw?³ß¸¼
{­?©3ê
0‡`?äe!~7?²L±øIÎ?ÈhŒts?¬TÊê+?ÅbbîJ°?©|©XZ]d?Ût¾àÈN°?¦=Î7sW?×cà˜9Oà?ªÄv¸8Ù?ÊNÁ
üÂß?ŸˆÄ¶Þ
þ?×ó7xE?Á¢Wšèñh?Ö>ôj~+³?ħ¨iÚÔ?Ò¯£]<Ç?¿¢
¤‹î"?º¸£ÆªZ?¼«Úñ 
I?ê;íá'Í??Á0*ïöP?³gí-5/q?«3ø´iü?Þ衎€
?´Ý°*"×Î?Ò×͊žü?´Íl;å?Ì!ϙÁï?­Ú7çŸwY?Ê ÔŽ°±?¤zç]ù"?à-Ásõ"?¶šâ—Téé?ҕ^6<'?±{銑¡¥MIXED4FGL J1545.0-6642?§t[ä°­ØÀ"ÃH² yÀ:L÷z€ÏÀ<Kµëæ@"!N"b£
?úÅva†,Õ?¾dZGŸ&?™p1ãŸCŸ?Ü˞":ê?ýà¸L7;+?ïöD_«aB¿ìáT™4¿áW'ÏQâK¿ÕHd]L·>¿ÃLu9_¿Øõ…ÞPضOTHERunk3FGL J1545.0-66411RXS J154458.3-664153?ëm¸.?¸tÿzVÚÄ?puW°u$?e%`$î?Âþže-\?¸#ÓûDxc?é—'Š™²ª?¾QKC—¦È?pÅI_ÂJÏ?zמ<`?É7ŠþÀ?½ØVä£-?í~}¤Eš?œˆ9'œ"¹?n=S÷™?`¨¸ðÉ–?³)üò'+?œ4Ò1Ë ?íñÆC=?''øá`2?u͂Æ®?\;ãÖµ?²'ºŸœ¿ž?'+·ä"[ñ?åéћW?ÄýWÞR ?‹á9´3P?rëõ¸Ç?Ó¡kSÏÏ¥?Äòëeîá?áãæl°œ?ÈñMRÌ´,?sOzÙ¾au?q7ULÒ²?Ûêöˆ«'?Èßë'Ål±?éŒÇáÖt@?®°뀉V?zº°)¥Ù*?p¶uìÄûy?È÷
÷2"•?®vÈ:?6º?èãÓ?ª¸á´?¬ ?…Wé("?€Ì¸:{Ÿ[?ʗì-û4?«Mƒw±LAGN4FGL J1547.6-6601?ä!w
<]ÃÀ"ì·M߇À:¤W‰SÑ8À<òÙ¦Ïã@k\æàÊ0@¥2.?Ézô'äs²?±óy^æ•K?é—tü+@áZº5Æ`¿ì"Ö@éÕ?ï÷_²íþv¿í°Ú'ÿ#¿Ô)ªžNµ¿ïþ;âÐ?ïÚÑrMû6OTHERunk1RXS J154730.5-655754?îc©JÍ? B'ÎX¦?ƒlcŠÔ7?€ñ‹~ß?¤êV©±È?œA‡î1?îÈH²\šF?ªØlgW35?Wr "̔?fÑH²v_X?¢¿äÐh>?ª;+߈ºo?ìÂ	¤2h¢?¢"þNqt"?Ž‹a®?"W'ü?¶OБ—0?¡imƒ›hl?ï{Qª(Y?sNÆ*(?lÛ6'k"?Wþ")ÕwO?‰ôÔ빨×?oUŽ×¡?ë÷ÆÕ´Ik?³ãéï©bé?¢u€dÞ3Ï?¡³-"ì?·	³Å?°GUþ	<?ìü@gpžñ?ÀF:l7‹²?q.ïB—B?Žò%¸%•?·
ÔÛ¸C?¿tÅ9Z"¡?é ÷¶§¾Ã?« ֐û"f?ù‰¶{g?'躭Õ)¬?żïîÿ–g?¨Œ×œèJ?îRڇ9_?'5*"8…?†Ÿaƒ@é?zäUùp?¢BùäWäá?‹P®}³2hAGN4FGL J1552.4-5612e?ë͏¢AUW¿ûöŸ™ÛÀ9Ü'³£0À:úZiØá®@!8X"UëD?ý¹á7½Üo?Á=
w}:?ÅÀ=\×ÇR@º.šG>ƒ?ó/ëb^?ïÿÔač¿ïèë Í?ï1}ñf®¿ÚTÁÔiy¿à&ǟ¼Hp¿æÞ'h#ÕÈOTHERPWN1FGL J1552.4-5609MSH 15-56?ÓT¿"1J?ÊÓ"5x̉?‡¶Ã82þ-?‰c9ÚCW?å÷!"½Pr?Ë'£š	½?Ñïºòs";?ÈÖbW[?ªAœFOÎ?©xgÃ"Ø?åd̽¶?Ǫw"Æ'?ÚҖº0è?²Ø¿³Ún"?µMöK–ïU?£°9@®êæ?ßÙë³À"?²³ðiic?¿™eä'Ãa?£‡;•yƸ?«:¢FÊp?›¹Ì+m?êY)Äý?«<Ì"Ó¡?ʃOà×µ?Âu
'²D?"9{F•2?"µÞòßÉ
?è½lÓE•i?à .ëó%?½ŸQMa?½Vq¢jß®?²çç}6¾V?º8å#Ü?éïíóÊ#?ÁÐ*áfH?Ò=Cµu~?°vý%ÖÅ?¼AbJøÌ°?¨¼×?ãY2-F+«?²š£6©Éã?¬C»êÇ÷Š?›êÕÈà3P?®BpÈ?§'þ"¾K?ìW¢àú›?®|&‰ZùOTHER4FGL J1552.9-5607e?ícýéqÁ¿ûÃ"›5{À7ª·Üz¿ºÀ:RŽ¨¤ÏX@ –=^…F{@¿Å¥'¡?«`Þ"J?µ(™QJJ|@È7 €=¨?ôý>!MØ{¿ä©»Þh?ïÿ—Ôú¿âJq=Yý¢¿ÞF™!N¯;¿äÒ,ó~~¿ßŸ[O7OTHERSNR3FGL J1552.9-5610MSH 15-56?˜4À…XÔ?•ÐXZz˜ú?Ðu0«/?K¥æq?î½ ~)?£oî<{¸?µv'ðeÞ?º**uõO£?׃¿3j¼?ǟ‡B1±\?áNFVrö?ÅüãÚÛX?·}Ôöâ«ù?¤Éqƒ{?¸",8R?¥tµ\b§?éÿ¿Ýó]'?®ˆ¾øEBø?©‰Œk"ÀÅ?‰­JÔÏ™?ÐnêÞž?©…¨¤ô?æY¯ÃÉæ5?«Äèéî-¶?žüÍ+Ó~©?œª˜1ŸO?žwÐøÔ³8?£·:™wîv?î[Í?¬"
u*#?žø:¹ºKk?®óeçJ?Ûߜ&€Œ?Έ¥B;±(?ápñç—?ͧFëÌÂ;?µµ»tÓ?¤€HTv‡˜?µqiKÌp×?¥ãkpw'?ê›h!«?°""­á?"'¦3¦­?~R/KiÚ=?Ò(€ÆD•?³ŽRWˆ?æG*É­2©?³‡±ZûOTHER4FGL J1556.0-4713?é™MâiŸ´@EUÅ.rÚÀ9F"'AiÀ;.…bªð@Èӌ.¡ÿ@K¼±Ì–F?¼ueáÙ?™:†¨j?܁M½£7?ä;CÖw#+?ïÿý{ÁA~¿á[?÷fÔJ¿ëwpåEi—¿èVÇ¡Р¿àãÕÈc¿Ô‡^ƒ˜üOTHERunk1RXS J155608.6-471529?ëWÏ~û*%?ÃEV:8#ø?m·Áí\¤›?r}
ŽÄ"r?Â)âýeÆÙ?Âþ§X|¡o?â!4sºë?Äq>Ê?«+=P°?¤
kûáT?ØX0JBç?ÂÑÎKIvä?ãí6"ÀŽ?µkI1ô°?ŸÜҠæÖ?'•ŽB÷—?Ö'Əé9?´àœÒý÷?ÝSÝNòxÐ?­£žW[–?¸+ïsÑ?–Æ"Ùúúá?Ü¡&ë&?¬wäõÚÚy?ç[°­‡b4?ËÓö6Ó{¾?'<-R7k?†Pq%"á?ж½<%{?Ëk-¾‡Ã6?ÏT‰'}ÑÆ?Ä/iî
í²?¼f¼LQ?»L¥cëü'?䞇×
¥?ÅC¦
§Ï?Üáà89'?·!xùû?ª*m~–?™xJ¥¦ÔQ?ßÙ¥o³
«?·'ÊVv?Éä
ƒ30?¨¹~jˆ?Ã÷ßµ‡¶Ã?¨IÕ ®KW?ä‰qÑK?±Áº`\MIXED4FGL J1601.3-5224¿ïL/lîڃ?ÔÓëd'{ÃÀ7øKZqežÀ9ÀBHyìU@^¾†GW@løÿZ¾'?Ã÷ÁÃuU?ßó†?IÁë@ÖO@¯óx?úŠ9\mT?ïìz|àP¿Ñ¾²m{¿èYüá¨I¿íhåf÷…Þ¿ëf`ۍ¿ïäèaþ¢³OTHERsppSNR G329.7+00.4?¶ë¥ÁJW?»A¸˜Hœã?ҞԎY–í?˅‰¤%†?ãí8D6ˆ?Î*üD«øä?¡~Ÿ–~t4?©#Ñ~RåW?Õ­']µè°?ÃE­Ö‰Ü?äMX+ä?Ãq«ûNÆ?¿›Jb"ŒÔ?¨Ë>_Âá?ÎÎñ«f?±ç¸Nï?äY7F#Œ?´±>†£r¶?lñ‡éW?Ø?Rr¥™¬`?ÐVe§"ê?©rÓ=FŠè?ç·Û–"+œ?©­*x	?°.ñÝöÞ?ÃØá^jW?Ð.–Æ«u?ɦPñ#0?åâÖ`Á®-?Í¡{¬/µ?†/±k¸?/Í­?ÖX"°j…I?Çq6üø®?ä{\èÁÓ}?Ç9>qøc?µÈZ?£ëCXºï9?ÏÂùV¿ø?¶"H€""_?å]>ànò?¸Ë³|­Ï?E¦~ýn4^?3tìÊK£?ÕD2[¿:à?·©_XÖ—?åX}2c]%?·®Ðn1GOTHER4FGL J1615.3-5146e?Ì ä(g¿å3X ÈÀ7ØÏä¯A¢À:o]Ø"ke@#.zìu†?ú#'ǁ&?²¶""Ý?º ~"¿÷@
\irŠa?÷œŠÂ¼'¹?ëWË-\¿ï";C¢í?ïž%"ôÆç¿Éf8ِT¡¿×æø<g9u¿Í)- Í›OTHERSNR3FGL J1615.3-5146eHESS J1614-518?¦'…þ;˜?§ƒê:Ëý?'hç¶bF)?•"ÌÒõ6?îM4H±õ†?«¡[•¾H?¨‹D"ÄÄ?µ\òܯW—?¹áÈÝT?¼o‹Ï½©*?ë;šâD?Á(lª<ø?¾Ø£ðŠ—?¨"ŽdÜT?±tè…÷¡?¢¾)0-£?éöNq/˨?­ö«OÏ1?¦m PÑp?)tóé™?¥ ‹Ò
î(?˜G3ã_Ë?í?=ÂG'? •Ö±#D?¨P_«ñ'Ñ?¤×"
DŽ?}Dìc)ä?'@Jè4s?î@p,°.©?§љ÷H³? ÐS!­;?ªµ‹ [Êi?µ¤Zyßo0?»³¬Gúž?ì>o~Šk÷?¾¿½3–t?¶n(
c‹ƒ?¦$Ý0Òm¼?§O¶ÃîNI?¶0ÞW)V?ë½?'"h?«nµìÒ?'&S¨}ö?ƒëS;4‹,?¥`ÒR<? pýïߕ_?îÉ­]›½?¢ÌÏKä!VOTHER4FGL J1616.2-5054e?阶ÝC´Ø¿À©ˆOnÀ6â1_ô\^À9ÎÒÿì´Ê@!®š‡«/™@aED­®ú?¡Ùt~Þ$?'¾#3-K_?á¡_²??ühˆ_?îï«>\²?~c45oV-¿àŽ·ó÷´¿à"pð›¿äÓgÁ¿×‹&ŸÇ±OTHERPWN3FGL J1616.2-5054eHESS J1616-508?"Kk…¬t4?ˆ}"&ÿMr?rù$ž¾D?qé[ u8?ï?²"CFÚ?Œ.Sz{q:?¡}i…|AŸ?©˜÷ž`?¹¸°–`T?¹± ¨4E?ë±&±£.K?½»-ÏÝ?Ÿ%z3Áö?˜±ªüPD§?•Š.vóÂÔ?kòTm?îZ'»í½™?Ÿ8`-l?°!;Ÿ·lž?–#¼¡<M?·û¬\ê½? Ú'¡¦Ì?êüxo¶¥?¥¡D|¿jÐ?—þkXÓ%¸?Œí&M`tÏ?rgÙáèÒº?pr·?ï<ñ;Û½?CO†¤?Äƒåîªð?¢Pí×w?µÏ'';?»Á5±µ?ìWéžÈ5A?¼¥ó¬ÏE?¤Þ,Ï_?"ȨÞhÓ?'º…©K)?‡ºéË`;)?î…ሓ?—=šh—0B?Ã¬Æ$Ő?‹MŠVÃv±?¾9½N?©¹‰åK½¦?ëN›b,×
?«­ÖÁpJOTHER4FGL J1616.9-2257?åç)"ŸMt@3|€Ç:¼"À:GOµò–À<	÷´#ì@<r¢ÿ@gy¦µ?ǔf'?Õº´|ª@Ú<÷Ø?üdî—!ð?ï÷n@ÐT¿ät<Ëbj¿ßÔ½|Lן¿ßͺ}¿ÉY¿îZŽâ™¿ïÿÿ)@k*OTHERglc3FGL J1616.8-2300M 80?ßGY9›ñÒ?Ä}oyVû\?×0G>
°;?Ãä*p…½Þ?ÿ²»æ?²º*ÖêÉ<?ãN•±…0?Êañ{qª?Ó6ÂYP£?ÈXgyz¯
?¸°IB¬ô?²hô$|è?âÿ\àq?²ÔL"6ny?ËÐ¥Ž3MÏ?¯g'k
Ø$?È1\þLk?©I¢—a^~?à>KcOÂ?¤L€¸×_h?ˌbÜ: \? }S •?ѽ8gN? ¡cùŠ×?×Ëw"®o·?ÂòQtD~?ܼŸ8ü2?û9b³d­?ÆïÒfÐÕ¬?¶_-èª?Õ(âG{t?Ë3fÅíò?áňc$?ÎR·@Ϻ?Á;%OÅ»?¹¯y–ˆ²?Ü¥l¨—/Ô?´RóP¸?Ô
§Î	c?´úé;£ñ?Ιו[O?°'Œ<ã?ÏÁÀ˜û¨Ç?£F"³]¯?Ô?†@~þÁ?®¤Mb]?Ûߙt
š?ªô‰LÑ\MIXED4FGL J1619.8-6314¿ìÕضSÓVÀ"‹<æÀ"À;N»"¥íÀ<¤$Ÿòy@!ŠÙb\k'?öhó ¸r?ÖuK[žn?Úû•!ººÑ?ù¢aôçž	@µ'§‡ÃÙ?ïŽ^g"cпíÉ_²¿êsŸ¿£n…?á¹O!P\º¿Ùâ`ûÈ¿âU1U¡ÏOTHERunk1RXS J161946.9-631530?îx"qÞâ?¤ìzü›S?fΰÉiõ?cÂÃڙ?§»½?£˜6
[¬,?玭Ep?łî	æç?x+f5ôñ?‰"£¼?Р6‡·«?Äà SÇþ1?ímёzÐ? ­‡ 
u5?¤´²Q.ò?|h"µúca?²—(']ßQ?žç·so†?îæë-ØLÕ?…c'¼ñø?`'ñc•à¬?SÒ xgd"? ˆ.Çn?…®|]QG?ëü$ǂ?»Ì÷:Å´ç?y'í¬n?tëËïòá?¾ÅÈC­?»FÞ.5?à€%À6™ù?É0vÕÊLj?zÛõËÿáb?o"	søô?ޔD§òZ?ÈÒuߑ[Ä?êˆVÍäqQ?¬ž¼@<Ð?ˆŸ##ú?ƒ'h"ž?Ä]ê×NÛÛ?«H™Ô€_?ì·ø>'@?¥"]¥ºž©?uä">»Ò?s·|âxs?¸ç0¾¶J?¥"¯°9÷¦AGN4FGL J1626.1-5904?åÏò¾p`À¢	?Câ®À:Ûõ ¨ìôÀ<ªŒ0$‹@ Xs~@©ñ…é¹m?Ãé§c†¸¿¦±€Á™G?è<ÓÅåR@ïÃåG—ï?ïÓýB¶]õ¿Ü¬3$D­Ú¿ëÓ	\ ¿èw~¶ß%¿Èäß¾%±?–''ᶶ,OTHERunk1RXS J162613.6-590658?éQˆ:÷wÆ?ºÒgLé?yµÓ« µ?ry[¦õY?Éì0uє?ºmõ«8Ü?ç'l·8eø?À"!ý=$?uiÓÓY2f?{2ÙÙ<'<?ЇBLÎ?ÀI7Lrt?ì%·‹¦?¤´%éa?÷¼)?xXüg¥´?½n÷!½?¤AªïR>Ù?îxòܚ¹ï?†øf+ù›?ZH
6 -?GÀùÌp&W?§ž'vƗ?†â%Òâ
ƒ?ä-¸šºx?ÄÊ]u•È?¤œ2úHô?…ßRÜ&ú?Ö·ié}²ˆ?ĕ¯¾
?ޗjɀ?Æð†˜éy	?xàòµ?‡ë
¸K÷ª?à'˜åOá¦?Æ«·^%¥+?çax×W?±ŠÛà—Ù?'âãÕÌ?"¢Úódž"?Э——?°ôšÇ)?êfÏ/'µÒ?¨LuÐ@é?w­ÖøÅ?p§0R"¢š?ŧT‹P3R?¨4jsMIXED4FGL J1626.9-2431e?×Bׁ—Ö\@0º{¢7ÍÍÀ8.ΉenðÀ:¾É'•q@ÅÍc ŽU@ÌՀÐtø?°ú*~å8?ºãi`/¯_@šÐ=š•B@oXiM¡t?ï¦qï0¤ã¿ÚðŽ•·¿å,¡^4׿äL-ráõ¿æj#?O§¿ì½¸ƒi¬OTHERSFR3FGL J1626.2-2428crho Ophiuchi?å÷£'%h?À=yà80ë? Ð4vòZ?–Á"'¥L?Ñö²\f»Ô?¿ë7ÜeF+?çËXÖÊ?Ƭg°?ǧW¸×*?êÓ¤d#?²YŠ¹B\?§>ý+d\Ì?äRRß19š?µ·`ʈ3r?±/ÆÓIÐ?¡E;Í¥S¦?ÓPr*·?³ð¹g\‰?ÛøK¸‡'Ó?§Ó´µŽH¬?½²Ý"ÍQ$?Ö÷ގr?ܚüæEä?©íÒ¬ºÒ‡?àÁ‡ñóÅ,?Ã¥…úÅn?§s\ôɽ?œðg²n?ێ"}'Èò?ÃÒ:H?༩w™OÙ?ÍOÔD¡€Õ?ÖÛñèæ?Í
Eá0S?¾ªìŸa?³:!ùt׋?â‰T=!§"?³ú˜æB?°gòw×'? Æ-qC°?ÖÓZç=w–?²Ñ³Þ¶¦'?˙îØT.D?£Ï3ie,?ÇJªâÜ?¢õ¾ôÍö?ãT7@;¸?¯¤õo»MIXED4FGL J1627.6-3852¿ïß[Öљ¡@²Y@ãõÞÀ9£.>׬$À;‡A©î{s@•Í`E@¨@ƒ}Îb?Á7úÃ*6µ?Àž}5ês?þ•Âú»óa@8þ'¢?ïþ0O‹Y?½ï¦–'7þ¿äAç`ÌÉr¿åYg°ã¿è›lØpnþ¿ßgÍÚmOTHERglcNGC 6139?çE÷mV¼ó?ÿãÎNµ£?¨¹(WÇn?Åi†‹?̹Ø32\t?¹öÿ'#?æ»Y4¤¢a?ÁdæMk1–?œÜØCߏ?"""Uv?л€xÂM?ÀtÒL¯l?ꩅB}0¶?§¢Ô©¶8?™¡9o9((?SZ\–$?Â%ÃÇH1%?¤óÜ'«*?èåuÇq2?˜${¥áÓ$?£ÒO'D…?|mìÓ¹Œ9?Çu•`U´?•‹»Š…) ?ÝÃfCxG1?œ×SZèP?ª+ê:Š¯?»m:»°M?Þ÷5ÿÉ×Ø?Ã
 |ŒÃr?Ü·­S¾K³?Å°N æ®º?­-{×
¤?°Fxío?ߢ£IåY?ÅÃkÐÀ?ââ⡱|K?³6k_R(Ÿ?°í>c;Y_?Ÿ›  i©}?Õþë#`="?±_¿$LùH?àýÇÍÎC^?¥åË'x?µ}¢]±Ž?'CÊ]?ؽÐû°?¤r«j½¾0MIXED4FGL J1628.2-4848c¿ãa(µ£2¿§¦{ªEÀ8ɦ¤D‡À:>žm=ðü@7RÅʤÿ@±y|ßý?ʦE9'ô?Ûß°i¿·;@'mŸ?ËÈ?ø2·bWc¿ïM:'£?ï­¨z-¿ÃœÏÄxëN¿étæX¿î¦\?ñÝ}¿áì!%êuOTHERspp3FGL J1628.9-4852SNR G335.2+00.1*?ƒÜ)>ÆA÷?"æî±Úö4?¨×r˜þÝú?©@dZXÍ?î#1`[q?«eÉ¥©\?žF‡9Iì–?£:i¯#Í?ÐG>
°:Î?¹Nr¤+P¸?æê,ÀÂT?¹WK[+s?µ_)‡îw?¢@‹õçÚ7?Áá"3•?ª4y"¢"?èÛÚ©¯;l?®ɔDVW?'$,Ä©ô£?süÐõÍ3f?Æ·#ö²×â?¥°íûÉú?éÉœ¿?¦ÝX†åóö?wk¶ŠÕ¬P?l\ÉÕ?ªå‡År?ª"ÈË7+?î"ЮBH?ª|…0²Î•?=Sí?•ûàäñW?ÑÀ'ϵ?Å+ƒFF
{?棱£¯$Ï?Äû&'åL?¬ƒn"iPg?–åV¡ñX¨?Íø0}Ì4?­C†Ö]9?éTK
·¶]?¯@´'M²×?tÓµ¸øÉD?`õæ–ã^ò?É‹Ð
ø_?²‡lùÜ?鏵 òd?²4wl»B OTHER4FGL J1630.2-4347?ïc–H½oH@	ƒÏ:eVœÀ9ÓT&ÈÁ¥À:ý¿;ÒE@ )f*×D@«Ænäº?À8ò9î¹1¿²ÉÖù "?óu­+FÕ§?þZ¿êU?ïÿu+%G¸¿èZ&–m¿êzÿzŸ¿éŽ!€Ù.Z¿ïá0œýç?ï"Ic `ÉOTHERunk3FGL J1630.3-43461RXS J163023.2-434804?йÉý?Èj	"v?wr¸¤4ÉÔ?v*
½©S?ço½ª<vu?È3rs?âó>HAQ?È3š‡çPÃ?Ÿ³;zV<¶?Ÿ=!s˜(*?ØO.oÒ?ÇN÷:oΫ?àRÇ ñ…G?²Ë)'?±±Â"E4? Éî^ã}M?Úî>a?±ã¤\¶þ?Û:ï
 ~ ?²®,^A?—˜»Èúwƒ?Õ"».?á¥ÂœÈ"C?²~q49‡?Êt'}?Ã\Òhî?‹3¡€r?7È$c»?év?Þy?ù _=t¢?ÒiüiXÅO?È£"ãîÁ-?¨w¨Ÿo<;?¯àPóà–?åC‡A…ää?ȗŠ(kÅ?×(ú-5ËÇ?±dzƋ8Z?´+$o®¶"?ŸæŽS+ú?áæ[F?²6ÏN»?ÃtÀ$&?«†Òs~?¡	–sq?˜©;'uV?ê=vûVo?¬ìtŠzô'MIXED4FGL J1631.6-4756e¿ïÝ@àšßë?Å>ÜIA'rÀ8;i÷ë^ˆÀ:,žh5s@#‡QàG}î?ü°œ!3?³¬
åpݎ¿›äÚ5+¨? ®¡>@c#ÃԀ ?ïÍÐmk=f¿ïý·áXJ?ïh_/:€/¿â;&a"˜Ï¿Ü³±ÇP·¿Ã•Ýað_úOTHERpwn3FGL J1633.0-4746eHESS J1632-478?œÜtK«É?×íDïü°?j`FöaV?n«"Ž|1?îþýýNþH?Ÿ•C(É?½xÀí+Î ?Äp²êp?ŽF1ê=3?—'hȖ\M?ë×Ï–?Ä÷¿cF!?Ä7—P¿
A?«Žþöjªï?²¤"k?¡¥1ÜM?蝉¨µÁC?¯~W›?õ?¶KY*Ô°? ‹7ô;?u—¥m€î?n^ÑpØ?íe¿«Ø? ¨Ñ5‹Sæ?£mµÇ?§Ý¢
–ê?jyt¿QZ'?t'%i·wÓ?î®­ª…$?©¬TkÃñ¨?¹²%õ˜ó?¿"‰ÔŠT?"§ÞÿõÜ?––'ãxß?ìwÅ$Ú!?¿è¼†Gq?ÁN6ž‹?©LK[hÉ}?«ˆ9
gÖâ? MJ÷Ð$©?éóîǞd°?®'"»Qn?¡÷Lþ
‡?G²Ñ`÷?vu¬û"?t'	æ}ð?îÂ0LV£X?'èpð—¨	OTHER4FGL J1633.0-4746e¿íÓql(ó?½Ü—Æ܉À6 þÊuÚxÀ8öÇÿ²|@ ìÒ1æ'@éÓHæ#?¥Ž
¢ÎÕ?®ôßô5¶@'Óh@bëà8du?Ü`àjcv?í¸Dµ;¶¿â_{l‡é¿â£-ab§¿äÜ(ŸÜSÓ¿âù ÀTnOTHERspp3FGL J1633.0-4746eHESS J1632-478?{'?.Õ?p¥O˺ª?\aô¢5íË?açáwh3?ﻢijl?ufvžR?•¯HT
W?£.ÊþyS?ÎÆÍÉí£?şP†ïã?ç ÒJ»5?Æ0¼sÁÌF?´$¥…?£ŸVôÃé?¦ëÚLDÚ®?›ï•…ªý¯?ìÀØ¢Ãå?¨Ì¬I?'ÓenJ¹?rbeÿÑð?­·û1:H?˜â—ögŒ?íÙ2¹e¼È?›þ7
Õ²T?' ËfK?x<s|è?mFäsù¼?jŒ¬òùô"?ïš5ï·Cµ?él+¾?ÅÒóÝ{Ô?®…l™Žå?Ï ãåÃå?ÉÂëÚP^?籘nÔ҈?Ê¿HăÂ?³NŽ¬Ô?¢yMáIJu?¨1í]ææ?šMž`¬&à?ì+O}Ûg?¦t ¶2!?oý Èk¢é?b+"Ý[‰?²s×ÛL+"?¢)ø!êT€?푇c®r'?¢Ã;×3UOTHER4FGL J1636.3-4731e¿ã8äë|I¿¿t Ù¬"À7:¯ÿ6¬À9b>G]@ …†× @t[¡çEõ?¬û&Qxm¥?»%A>IøÙ@Û]9—?ÿ=lP‹3?êv?ø="ß¿×Á±[Xp¿å9‡
Jݿ䧤WÚ¿æç: ã$}¿é
ŠA·ÛNOTHERSNR3FGL J1636.2-4734SNR G337.0-00.1?{ÄG+†k=?sº2_[Ç?sÀW7>?s¾XU*£?ï ðpÉt[?~öož"»?Œï6%£J?›wìå_Úu?Ω䨿/?ÁdºñdG?çã÷±?Áx]ãúªš?§ÌÅ&Kl?›boòèQ?´zó|€Ì?¢nº/×­'?ëóÕK;?§g?ÏS?v
'†Ë Ó?\û¾Jbc?³(†5RŒ?"¼´s1?ínÔzòv?"Ó낣™?zÕ*Ú×?sÆÎÛð¬%?v7Œ^G³ô?t&ÏÏ@¯?ïæÙf?ô"ó)Ž?'æK22I*?Cò'(@?͸p??Ä>¸ç+?èFd÷·˜C?Ä÷r#F?¦¤›Ú€Xo?˜'3õ(u?³oÍ©î0?£Ý™Õ|êN?ì'ˆ"þC?¨C+~×ù?Xº¦ìÍ?GÅ꟞
'?¹\¥'Oø?žé¯zòj?ìÈOV²ó?Ÿ'ØÃoÈOTHER4FGL J1638.5-4657c?£õ+A6¿™¬.FºN›À7´Ñk—ÿÀ9*OTÑél@ ¹ñ¨ÏB@H½Þó?þ?½¨K
DŒ!?ËE‹:_e@ŸwÞ]îÉ@^ìJìbi?îelZþ¿ä(05Qñd¿âý™ô2l¿æRɛ¿ä‡¿ê²á~µ'ž¿ïÕ)ÝÉõ,OTHERspp3FGL J1638.6-4654SNR G337.8-00.1 ?ˆUAö¦'9?'t×ü¬g•?¦F¿?s?¦³MŸÆ…?î:?ƒ°W?¨ó4^)?¤GN«@º?­‡ë¹zt5?»mÌ6Nñ€?¶ã€<':£?ëMюAe•?»–î՜eb?¸ÝoÐ9Â?¦Baÿmk»?Éàm±'æz?°1þ´Íé?ælBEAJ?²ÊÞpÝ9Œ?n¹âÜN
'?YŸâµ¡Ÿé?žøâ÷¨åß?"•gäHr?îéLM¿?†1[À槤?|n¥3œJ?qíHiçu?³o¤³Áœ?°,¹À'F?íY.÷<?°Œuٳր?"|qV¿?ž""&R?¾9Œ­fÄÊ?¸Æere'?ë R†ñ²q?¹¡äŸZ…?°Ó¢WÚç«?ž/RڀZ?ÐL1Š–
?²\dS€ts?å¿r챙–?³/Änx?MÆ4ë¨<?A҅_¸òŒ?¥2©³]´?"™gʳz¾?î¥cוӑ?"Þ'*1ïÌOTHER4FGL J1640.6-4632?áy'ËçA¿•aÛížvÀ82]œ"IÀ:n­2ӑã@#L¥)DÇÛ?ým  ôØ?±š!(ïl?˜Aä&Ìn?àïJÀîr9@	'™oþ?澖stkã?äK'Iñ»š¿àsuã±ë ¿Þ_ÂWÿ¿áLʳíض¿½VtUè>îOTHERspp3FGL J1640.4-4634cSNR G338.3-0.0?º2	õC°Ñ?µܺ"È?Îò¦W†?"	¿å/?ìr'ö·NX?µñ+ïА"?²lÏ"ßËO?·ïK¤Ç‰½?˜ðZ;LìŸ?Ÿx­<Ý¥?ìêãJ˜ñ?ºOx"Ñf:?¾‰«öúƒû?©ïådFœ?®b!^ÝL?¢TéNSCK?êH©&>Œ?°x[B¿?Ȁ'Phçå?§_øŸIÂþ?¨qeíG?'Ì]#75Î?èXű?©Ï–í?ÀASX'ðp?³û–½å?ˆØBu:?RþØø$ ?돋ÉLd³?µ=–‰Oè?­Á㻀é?²Qkø¡'á?˜²÷wE\?¤«HSÙ0?í^Lԙõµ?µìÞ[²±­?³˜p›:Üß?¡È«l4Cš?¤LŸ©ž·u?››¶É8Z?ìH'òw]?¦÷Nù´Í­?³—¿-³à?ž@¿¥×Fw?°‰sÁÂ? ¤`dQh?ëŒ
ù"g<?¨%G;‡¸OTHER4FGL J1641.0-4619?æ *®ý¯?´J b5ª1À7rÀCQŽhÀ9hÞZ"Ê@Œ‰G.=@•&§3¶?±B€Ùfè?Ã%>¨Ý.o@¾Oá¿£@ø»h {?ïþ/°Ç³ˆ¿á°"Ýz™ú¿âžÝ¦8äM¿æ…~†T¿êDûbÓ¿ç|VÈc±€OTHERspp3FGL J1641.1-4619cSNR G338.5+00.1?€ç«ôݱ?t,Í­Ž>U?'E¶pÿlh?•
þ&Hö?ï-z­×On?–ίˆÀı?œqT¨e?£="{}³?Ǚ\ªG^0?·ŸÙ{Ô.7?é6 rˆ«?¸úú¬«†?´»|¶gŽ7?¢3èí(ˆ?È~¤@¼;?°Šenµ?çHçY.ß*?³'á,–'?~^1@ ?eEêPYtg?±.eŸ}D‹?'OOOqÎ?íwʳ(?"lÈ×Ôû‹?w†Žƒ ?oŒ#§^…? u´9½lÜ?¢´ uļÙ?îʇ:/s?£'t¤E-×?‹yýÍÒA?•Gä2S–(?ÉÄhNW?¾ÑÎ-8â?é þj\"?¾¥Î!I?²‡P%_Ë?¡¨VuXè?È¡
(oWH?³Tˆ—ŽˆŒ?ç†ÚL¹"?µkñ‡"?`Öv'ê?QEú¡¨N?·6}·8©?žFo
?íYÒsÀ?žÆs<aOTHER4FGL J1641.3-5945¿´l¥ŠÊ'À!›ÿCAžÀ:Jœúw*À<ëoOC4@UbPW0h@úp#~ŠJ?½¹¾'B?o3§ƒYi½?¯)9£P@I¤µ¬t¾?ŤĚúÝ¿æoû:ža¿ã@Ï_~¿åÐx=~e·¿ãJwB+ɇ¿ÉLáłU°OTHERunk1RXS J164117.0-594647?îyLYlOV?•ýtғJ?iF<­*ä?Xæ÷$Í?¦ÖÖ¦jbt?"·9æå?êôa«Ž3?½8›OãS?`÷X¾Õþ?fy	u"o?Ãê›ñö?½ZµØ?îce3ò‡?'¬É¶½£?sš»Íáù?aWwþAÎ|?§V¶RzU?a>W€NØ?îö˅ÇL'?rÆ<:=ñ?b8ã/?ABh2'Œ¹?žßŽ&'Ê?ræ¦äà?ìî1݃å?®¬ñ£j?€4׶Rgw?qï+¶Û?½AówRê*?­"Áð²?ä™
vŒµl?Œ!égjÑ?gиÉIZ?xß|ڍª?֞Jûž=æ?Å}\ÂMÂÖ?ë7·;ëés?§'õ™HÀ?‰áxLå-c?|¨÷Ý&=?Áƒ‹'_?¥ísNjìê?ìÍ6º&W?§÷ìŸÌ?{Bá F?d»ðÞ.[ù?·âƒq†?'ŽB»uéAGN4FGL J1642.1-5428e?벲ђÉ
À¸ñ.ñÀ8ãíóŽ¶À;5@qà,@"¸	ò=@÷`¤……æ?ÂApã—êm?ʳ<'è'F?ýÌ–›¸X@cbezÙ?ïÂä¾®&¿½ûå~ŸmC¿á𯕄a#¿éikž´‹¿à
Ýað`¿Æcê
J[ÄOTHERspp3FGL J1645.9-5420SNR G332.5-05.6?ë‹ôË¢?°Ï½ò|?y_ŸÉ›¬O?o&»Y ?Á/Ó
G?°‡†j¿p×?é"‡0,æ?¾ë(Jª{È?'´³S9šú?‹#ðžXÞ"?ÈÖ¢®Á?½ŸŠE1Z?é¦#Ð60?­'	ÉÌJ?¤­#.W¤?›(´Ÿ=U?Ä<^¤"ä?¨,¹TF""?êÅÂàöá"?™&E¥UÙ^?™ÎÌQ2ê¼?x­e©ªZ?Á¯ñY/W?–ÿZ÷h?æDEoZ×?¾r‰µJúû?'¤dþÑ9–?‰À´æ| b?ÒM/¢s̚?½Ò12'™?áIJ ®™?É£#Â8/ƒ?–ð—U'EÍ?Ÿwo¯¹Œ?Ûþb‰À'3?É	A¡yї?â7<£…'á?¶ÇgÕs²?®Ëޝ&8p?›˜e"TÏÌ?׸
äƤÑ?´ÚDÒ¿kj?äI$Uíâ?«ö¯ñ»=?¬ú<ëšw£?'-Ñ@ò0?ÓÎo¶éƒ?ª­	{
nAGN4FGL J1645.1-3323¿ïÃ%(Ùh@ÇäÅøÀ:b/‹ÞÅôÀ;ÇŸïôð@Ñ¢'dì¿@Ayaë­c?ij»¤†]?œ2EfUcN?Üq°œj"X@mF/9?ïìáxU¿Ìp~WÉÀ~¿éšÁÀ	¿Ý¾Ùå9*C¿Ük
…?›¿è\v"œ;OTHERunkAT20G J164516-331816?êcy»`q?¸™é"·Î?pfý&ê?bCé]Ut?Åñ&àáÏ
?¸nlj?ç£Ù½1_…?ÃDZSnÎ%?†1.‰êi?‹K©Æ"?ÐæàC?ˆ|¥U?ì=ى–
À?¢Œmm3±?ˆ^jˆA?ê0´Í'w?»fqN õ?¡!4OŠND?íky–wƒÎ?ŠÞ`5W¢?qª+ý$Ԅ?T÷Ø鹋2?³‰Ük?Šr¤‹…Ǻ?åðkç·?Â<ßñå™?""ÕЕÔ?xõk¸›ù?Ó~‰¦m¤?Â?µ{* ?àìKµ¶ß?ƾQðžÊ?‹ìR†ÝÉ?˜hø¾¢z"?ÝHA»?Åîy‹ÃSc?å·hnuËÖ?µà+p¾{s?žÒû?'"íuã?Ò¤
cÉ[²?´œOTY§?èZJ!Èbì?£t£Ï9?ŒÚðsgx?w¼1W'y?ÌÕ©Êê—?£QÞvÆÅrAGN4FGL J1645.8-4533c?î#ïlp&뿧.€_ЎèÀ7Г¨¾Ð‹À9zc'ŸÐ@ê¶W?ö@DV;u÷Ô?À`"•N?ÐÈá°´"@àÀ_?úål8br?ìVP%"õ¿Þæ[L
¿åƒÚ_Ý`C¿éÉÇÄ¿ì/_i#¿è™¢¾[oèOTHERunk4U 1642-45$?ˆeÓÐih?†Ì|ûGš?gÒpQ?™
EQŽ€?ï{ÕI¯2?žn ×'W?¨¾ÊÍæt¶?¨ØèzW~?É@ŒžDµM?¶©Ý±4?è#ð+ka?·÷²%êf?´ð@"?¢'RI0È
?¶¡z—("?ªÕß1]­÷?èϙŸ	+^?°­_¦'?wcúzSß?aHÿ^'O?¸«i¿"?™,}m†C»?ì¼wcë|?šQØÙ®.=?q……Œ!Y?iõQŽÝÓ?œµ	ÍäBî?žšð~$??î÷M|¾>? )LŒm¯?'È=4IÇ?˜T¢h?Íè ÌS?¾õæeLœ?è/Ãæãé
?¾eOSéûÌ?­)—¿TL?™Ž2:îF"?ÃEzÀ\ôD?«słRA?é\ÔEù?­q›_…"?VÅ]J"*?HXa»yŸ?¿ô}¼ˆÝ?¤^Èy‹D2?ëö
™¬Ë?¤ƒõ§IvOTHER4FGL J1647.2-0154¿ï÷K²·Î@:T;ÄÒ,ˆÀ;üè‹+À=»	h_@ wɉv`Ú?üó÷é±	"?ؕ";ᭅ?ïû³ŸÕý@ÏE™›@¥"ºÔõ¿ïÿÿ" 5•?ïÿò> w?£	1à€fu¿Â"ÏÅЄ<¿î/é¿ïÿ}e†mOTHERglcNGC 6218?Þ°b¿¤Œ?Ïf±MHí?юqßã¢I?Ë,^¦9Ì?ςVÀðºW?ËÛ®Ã]ž}?ÝpŠÂ[B?δ>\m?ÝI2e¥B½?Îɀ²B?µbo?ªÁkúâÐ=?ç'ÿìê`?±•ÑÑØö?¾'»xð	p?©Lœr´Ië?Âà&'ÔQÉ?¬',¬»@?àñ݆%?´åc íx?ÙœÕZ²?µX»+Zd?´Y_S´?œb™¦L?ß8.C¤w?ʦ²NÂ?Óf=—÷>L?Ȭ)Øo\?ÊÃ(Jï3÷?È«Wéî=,?ÓR§††?Í`ÈË?âÝqªp?υʓÑGu?¼ÒDÆX"l?´iž.r½?å÷­"ö?´·¤ã–#?Â{*PØØ?°jíÍy?Ŧ7_›N®?®…ì6Ì$C?ÐÂbn<Ò!?¸-|©¸m?ãfR~»G?¾ M+Ɯ ?Àáñ#e­%?­I‡çÎ,ŠMIXED4FGL J1700.1-4013c?ï™ønçu?ôãŽ)ùΎÀ9+©EGÍÀ:´Zøt"@Ä=®·8@@›ùÆ*?Ëq†Àyt?àc!m8¿@âÊÿm3	?ÿEÚdåÝÀ?ïÿô!O…ú?Í°:ˆ¥Ö¿àý)áпö¿ë.ª¢ÖY>¿ébߓxî(¿Ýs—ºñƒOTHERunk3FGL J1700.4-4019cNVSS J165941-401121,?ÁøÜ	֘~?¾fj'ª¿²?°€ÔÂ3?µ±Éžì€?é~çmJû?Âûà-=¥?Ç31Ó??Äõ¿Vº?Çl^Íì?¼_i©ß.q?äl/p°í?Æpžgü?Í|hR"•?¯(₃·â?¿-ŸÇe®?¦|¶Õ¶«?ä»2Hª¥?±…n	5k?¹'ƒ—"¹?";ӎߋ©?Ë֓õëª?¢¥c e?æyççI??¦ÌJ×Ô4?ÁSÔ{Ë[?Á®Uwo'ø?´'¥Vü?¶®"'ÂÚ´?éºþæqÜ?ƵNbÛäº?°Ù$%Ҍ$?·Ã&"?ÏÈΪ6c®?ÆgcµBS?åò§Ðœ˜°?ÈN7{AiØ?ÁžD»,"?¥ b2:"ð?¿‡'·Öy'?¦RÆÉÃüñ?秆÷ÖeÓ?®ëŸÁhúò?b‰'Ö?âÿÀÊGþ?ÎÐ4á368?¯¹Èdæ?ç`ÞÛ5#?°·í[xÒOTHER4FGL J1701.0-2617?°W0Mn«@#Q2rC{À:zÝì¯ÁÀ;æiŸ
w@o=O–Á@Ö3Îc¥Â?Äóöû‰#?Ä
‰w¹?üv[ÁǶ
@V^Ä0›ÿ?ï	GÂ6pÕ¿â
Fªß<¿èݘ—;ˆ¿Ö&ˆ_µr=¿é"^úŒN¿çAÀ>ÉêOTHERunkPKS 1657-261?ëÖ刖£+?²æsEí¬?ŽÃÇÚ8‰ù?ƒ@6Y‹ë?½pZÂ)–ã?²p¿z#¾"?ìÎ
.N"Z?±\Zœ·8ï?'¨õó7?|-Œ(åuê?·:«ïfèˆ?°Ž¿â2Ù?í¬sÇ*ª?™xŽçKï'?‡Kåô '??}ÿ«ï‹T?¯eÊuqn?–M
h
?íh¢Š•+?·Ê±½po?Ž]Dy`[?gsw•¤Æ?°ó²hP?€|k‰Y'1?恬(£žf?»œŸ5åÀ?¤è‡wßß?œÅ¥$?Ðz
ž¥®6?»*—²}…?莩·°D?ÃuX3j2?— •
·?žÀT}â'6?ÊáFrf`?–dr'»ü?èÁïGºÃ?¯¾ËR/j?¥¦N‰«?š.x…ÅÎ?ǐd ­Mð?©|>͗¹J?èÜØؖ&?™Í'"4ß?¥kè30b?†Öž"ÆŸK?Ç1¢'‡HÖ?™t››B	gAGN4FGL J1701.2-3006¿Ã+]¼HÆ@Jì$·oÀ8©2ëƍÀ;"'>E@V.?ÿà2Š–ÇW?°1§—ß]?؅»@]h;@&ÇH!Äv?ü^ÖDoƌ?ïþFA'×5¿ÓP&žzT¿ÝBã_5o£¿ä''wcå¿îɨ G³ž¿ïÿuᮆ;OTHERglc3FGL J1701.2-3006M 62?cÙSí·®Ñ?_ÕãƔG?ì$RÎ6¸?¶Nӎ;°?¿PÉӕ‹?¶®{Yç?ˆ(xó×?—µ·ëï<?í–'¯H?³®T³•×?´^M;'ÀF?³'¦xR·?‰—Æ6®Þg?…Þýb'"À?ëàbèq\Ó?ª.®¸;z'?½ÉïôUc?©[("ñ?‰#›<fK?pêù²ÚÅu?ëB1¹i ^? !áæµ7?Áevß&ãç?œ	䧬NJ?kJ0T£q½?b·ªñA¶ƒ?ì*0ŸóY?µRÔX?½Ô-åғq?´ÿŸ-Pqè?€c¹"æÅ?'˜ÏNš2j?í4Ë'Ÿñ?»Jðvª?µ	âuä/U?º¤¥Bš.?âÃ÷îû?}íì¹È]?ì¬ÉüÛ)Ô?ªsÿ†Qv?¸]W˜‡Á?©b¥=q£?l¦ùú~
?VìµÕúDî?ëM/â÷?¢-Ú×!±?ÂXïZk[n?¡ò
R,PSR4FGL J1704.1-4140?å<Š+ßÏ*¿Æ᳤1ÎÀ8à8¦À:æ5SŸ@ lZ$c·Š@<å;X›£@ÏÓ¥."R?à/SàQäÏ@îÀrKv÷?ý'Êß·¶?ïöÉ™"{¿ãïD[y£Z¿âµj¿'{¿âŸp"§Êµ¿é¹ñÞ&Ò¿ïÿ2z¦KOTHERsppSNR G344.7-00.1?"""Îrÿ?† ùvƒQõ?·Yª'íR ?Äs®3À²ô?ìÄB— ºØ?Ä{'
'm¥?µù)§]?»<
a½?±œ³^—?¶ÝWœÒ'»?ë
Zz0.?À‰^½Š?¿¬JicN?£átBªÆÿ?ÍklæïI
?±Û·^Ì?䯛y¡4K?²C°Rõn¢?¥–«"?{«ãlM;?Š *NÕr…?›s ®Ø7h?î<¥ìI{?¦éQ"|Œ?'/·Ֆ?ç! Ö?´1&Ù&°?ÁΏ'û7?í1veôç?Á<aSÆÀ]?®=n
¼Ú?¶QpØ¿¦?¶ÿ°Ö Uã?¾Ú³Ò¢?ë<3—Çæ?ÀMÒ¢5Ö?º}®ˆ+?£†ÀvîB?Ð1MÙq1?³­m¬˜ß;?ä§)]­–b?´€+Ì´?¥¯LZíÁ?­½ä³"!?Šáµ#'ÿ?ª‡Ö¿éS?î9"eÕÇÈ?³ÞÕ+ù«OTHER4FGL J1705.7-4124?ìäۖ$6¿ÑA…±ZÀ8q=†ÅÀ:ÅÒ݈@NQŒÂ@]lÝxì{?ÇñPå ®6?ˤK¤C@Ç@ˆ…ZGt3?û½-Dܨã?ï­tw¡!M¿Íœñ½Ç÷%¿åÈ
L4¿å@@aïß!¿èê'Wގ¿ïù+àŠðOTHERsnr3FGL J1705.5-4128cSNR G344.7-00.1?¨êŒ}Í?¢ë=#—¡×?žQ䧞Ú?›"¸…ã?í~Èäð@?«gz֓}©?¶·N|?²?±·#–?¹6ã Ì(b?ªG{ŠR
p?êì¹.èÔ?µQ†]O¾?¶¤-²šæY?¢¯­Ü`'f?Œú´å?ª‹íQÔ=?èˆ;Âg²Û?¯²\\Í;?¤Cµ¯¡Y1?ƒ†pþâ÷ñ?¸]Â]E?•û	ù?ë°YŽÜ?šMD¥x)o?—r²'™œÖ?Ži¹ە…?›š·Z{C?˜Ÿõ2¯p??îg"µóÜ?¡_Cp7ã?ž¯uQ		? 3aCén?Àwº»l?µþ3œñ…?ë&´["?¶ì=Õád?±"7KŠ†Æ?˜à­Ÿøè»?Äz¯hãÄ5?°%P†%*?è°Í<U¾?°¯ú73àè?ˆrÉó"çÍ?qžZ­l?»d|¨y=?ŸÁå×Ïy?ì1¥BÞæš? C×òÏþ¡OTHER4FGL J1708.6-4312?ƒ'2¢&¡y¿ü4 HtãØÀ9¥tæXÀ;æñ;A@'2]jÔ@N¿ö$µ?ÍI>7s3Ô?Þ8ÞîãM@YДØ@°{/Ì ?îÅ&æÖ«¿ÚWq S²…¿àºëÄØí¿ãÂ!­Ï±"¿ïVNád‰l¿ïT?‡ÕK÷OTHERunk1RXS J170848.0-431418?«x
¸¹?¢ùV0«r?½*jaȝ?±Ö Ýæ?ꖚŽ|?µJ"hZ‡?п\êxã?ÃZUêuÝ°?³5jŽ÷џ?©ëß7©Ú?å9¤¬GF;?ÂѦêÿ¬?˟ÌN!Ì?«>®ØÄG…?ÆAÅa.Õ?ª«¤uJë?㇩{¨±©?±Oœñùé!?Â|c;AR8?œ
ÖráöŠ?»­Óôo@?—æ¶RÃät?çë,²I+?¥aÆßñïP? ÞP"!w¢?"FïäJ?»²'ã|oE?±–ÜÎ?ë{ÕúÚ?´Ñ°@·ò?´*ÛÀ*‰?±ËádÓL?·åk"Ql?²É´i~Ÿ?ê˜Gڊ$²?¸FÓ"ª¹?»"˜]?¬Ó÷Ó$š?Ã膧#šå?¬ü&@Vh?ç¢]Ä<–š?°PÊèƒýõ?©8‡mãq?Ý´,–+¾?¾4%ÛÎ?¤¡Ñí
>y?ê©qœiO?¨$2¥žÔzOTHER4FGL J1710.9-5247¿î`{K-ƒyÀï•·UlÀ9þ¹®âÖúÀ;'óá
Ì@N0Üêù@ÞÏŒ0û?ϝ^ mÿ?ÖÔìԍ@ð¨ß‡ºt?ó?ƒ3є?ïÇ:"ÀÅ?Øá=\¬Ô4¿å0†yÇ¿í8⟜é¿ïÿú Âî'?ïÿjÿR[OTHERunk1RXS J171043.7-530019?Ûû%r!ÒÛ?ÊÖ{(,?¹E¸êcy?ÇÓ@?œ?ݳlR}j(?ÊXY7© ?Û@`ŒvŠ:?ÊI˜b"Q?½Pëû܍?½–¼3fM¬?ÝkdŒ
~£?ÆéÅX0»?ã:ê%E?²[Ú΃‹Y?²»±%å2m?÷ê"YÂ?ÔÜñ— \[?°°eõ
™Ø?×*]iÆè?­0$ñ2$?Î}è]?ªÒdnóy?ٗ£>ø¨?­"­'ˆ2©?Ñ'÷7Pñ'?Æt`5[Û?¾Ã®ãO<¡?Á°ƒbd?㓎‡íŸ«?șN6ûü?ÇÌ7þ–jÝ?Æ:
Vh?Ë<'rç?Èqo_oh?ã=Ñ|xî?˶Tè\Ï?Ú3\	&€"?°û'Ƽ?ºö˳¶?£VÂÜî^ì?ßñ/,¾O?±ÛžÍ5%?ÀX¢-çÅ?¢p`ŒÉÙ?Ó^x
Ә™?·~쁡ií?â:¾R
¹Â?¶³2ºðßÚMIXED4FGL J1711.6-3407?ïo+A]@	"Äv£ËÀ9Ÿ6'Ú9À;$É:q@vŽôÏö"@¦NÜ%´?É;Û7ôŽ?ÉxրÂ-@¯~Þ,q@ö™ŸxÖ«?ìÚʆ¡oQ?îÝIúÑÿãÜÀ•†åb¿è`´á¼©¿é/Q/|¿á׊`@²xOTHERunkNVSS J171151-340701	?çØSӉ ó?¼ião6Õ»?¢ßâ#,?˜q{¤Xgà?Ìîz¾Úh?ºÐzÁ½$8?ౘÈՃ?ÅÍôGÖ¡?µš¸'–
½?²QLW;ž?Ù6!­­Ul?ÃB³ìÂ?âÞðAWI?±=»~²Ô?ªuŽk—Í?—¯ZŒm«?Öõ\]gÔ?°
¯"i;?ޟæ[$z?§X80‹°?¾
þÓ&¥~?›deÍg»÷?Ùܙð܈?¤ð!Åàdþ?×îob(>?Àl!ÄÔc?¼wÒÊg²?°]}Ù{…'?àyÍõ§ó‹?À_â%¥E?ÍrX`h?ÃB¨Ö]å?Ä/h€ûp­?¿˜¦Þ^?㗞‰ºË»?ÆXþ²*½¡?ÓC¡‹¼f?±p«DÙý?·Æü,7 ¾?¡}C!½À?ãeO´ŒþÅ?±Ô-–ˏß?ÎbI¿DV¥?§†"8dB?Å3ë{èj?ªÀ> ®õ?ãrɏð<?­¿-Ï\yGMIXED4FGL J1712.5-4642¿å^kò'¶dÀ'^!ôGÀ9˜ð¹À;)Y•Œ@°ìaŒ@ƒxÅä?È¥©GÎ÷?Ü'q~Gƒ¢@óg†!Ñ@¢"¾"y¿×|z"«uå¿å}IÔ+¿çá~o¿é€kà£Ä@¿î""¼ÃjM¿íú¾z$OTHERsppSNR G343.0-06.0?Ê͕~g1?¾˜ºêø?ÍÅòT¾Æ?¿-ÕPT]?áÛ
pá?úuý]8j?ÔáHÊ^š?ÆsðûÞ»À?º2gà}Èr?³È-Ö9ùo?âIü¥?Ã};
5?Ø>ÿñÏf?´Èò£é,>?¼ÿL2Õâ˜?¥³°=—]?à@–ï¬[ú?´¿MÙãÇÌ?ÄÉå;Ùu?šiòŽ²½?ɯE?Á?¢¥§&ǀb?äŒü6`¨ü?¦ÿ¥4~ù
?Â<[m?³'ŠŒ5'ï?Ǒ稠"?»_}OGL+?åŒovÒ¼?Â1l->–X?¸FôJß.?¸=ºtLÜ?Äx7UN3?Áéwy'™?çØú(`Øn?ÄD¡¼ö"?ȵ&ŠOÇ
?«ð_3?¾3"Yôñ?¥ós•þù?æEÑ£ÿ­?²'œ\À?¢Sûâ†iÞ?"S'ö»G?Ñqe€ëÖ[?°\™?û}?æ"
ö?°.¡nžEOTHER4FGL J1713.5-3945e¿ÈÑ@"²¿¿Þ@zcÉSÀ7aÿ¨Â,À:fpÍÈu@";@1ôD?ùµ *­R´?¥#Rj†¾?°Ôñ‰o«@aw]?÷Ž²Jj‡]?ﶘ]Ywk¿åہ›v¿ÐŸv¼Ï)¿Ñ?áAxñ¿×Ś^:á¿Ô…·eOTHERSNR3FGL J1713.5-3945eRX J1713.7-3946?Ÿ†ò'?§žF¯?ÃÖtzj;?Í"Ne¶
?ê+IãV…?ÌÙ×þ•Wý?¤^î!7?¬ÄPïŠ%®?¼Ot-4§¹?·žcØT…â?ë0"™KÚ¹?»ãX:ºÍ,?¸"¯4Ú~ñ?¦°v6à^F?¥Ìz\0=?œ®*P?됢s¡§?ªû[漪C?±LéÂWÒ?"ÔE·3?²g"B½uß?™¹o
Y"ê?ë‰p?"PÁ?£°6—öê?¶Hô¸©Û?¸–!ßH±g?¡Qۓ.Þt?³w"¿¢Þ5?ì!ïË<Ý?Àò0*ãX?™R®¡ß?¤Þœ"ºÍ6?¶þÝsÁ¡?ºn†ôÁ€?ìt¯qó}?»æçPí¿r?³6@œNëü?¤è¼Ÿ0›ú?$v]Ӑx?"yrYO+Ö?ì°9•Dm?¨í{?§»?œ¥Ž1–?‡¡˜·3—ä?³S_|×ù?¡VßôgˆŠ?ì°gžÊ°é?¤?"JOTHER4FGL J1714.1-3811¿ï÷&¡™1.?×5Œ	À8ÃÌõçxJÀ:ºæç*F%@"/ÊF_µÈ?ÿ %9um?»"Ci6Or?ªé^ºS+?ñ+E"ˆ¡@}:«w'‰¿£™1"́þ?ì¦a
¶ø¿Ðþ<[zû¿ÝNjܗÆ¿ß/Ÿ•\7¿ÝR€*‡¾OTHERsnrSNR G348.7+00.3?À€=¦Ï?¼¡üT#î?‡5«|}Ñ}?"ƒ<Çæˆ?ëƒVÈ?½dÝØÁU?³—Œ(Ö/?¹Žvˆý?•סÏä}?—KwUT£Ï?ìä?ÂZ$†?»)ŸÐY8?ÍTNùõœ?°ÌãÓ6ŽÖ?´i€
%µ?£Îôlãƒ?æ¼[t'?²'¿"fȑ?Î_ÒOºõ¬?¤vÄc×z?£°ízð ·?"2R>7‡z?ç,ü"Tz?¤Ð!ehE?¼B¾¤7z?¸š±ó\Ín?Óõ2F¤?·ÿŒAá?ëñ$øv|?º"š[¿?¯îº¨€?±,ظ–É€?•¦­™ÏÌ?¡›0ÌpN?íSÞè"d¸?´1‡´?ÃCN…rg?©ÑÀíê€q?²(¥&ä?£œûê?Ñ?èêº#Ä?°qt§ëÒ?¹Ù‹a~Ö?š½vºÜ?¦âj­mÂî?0­^ã†?ëV§è¢ýW? ÖD¼9ÛOTHER4FGL J1714.2-2928¿æȜ\Ó¦Â@¥w–9'ÉÀ:Lp–À;"7À`­À@"ò}
—´@
ˆ~¿"À?Ìéÿb¡4î?Ù
°Â«
Û@—'YY7ª@µ2Ò:J¿ï?Wc"$?ïÿ×á¨Ññ¿ä¸¯©¦W¿âá4bÞª¿îa*ÝyBa¿ïþ]~
qôOTHERglcNGC 6304?Ù¶‹lÛ¡?ÄIbƒœ›ñ?³yä…Ù¦Ø?­¤XÏÏá?àµ}¸'ƒ%?ÅZ•š(H?à(3¬;?ÄÄ¢^¼$?¹E…³°1'?°Ìý/|U¢?Ù^7;^-?ÂõMn¦Y?âPL˜¬V,?²bS,£?¿ÑSž|q/?§áú`T?ÓkåõVž?°Y«,"´?ãN{~"?¢P`éÅn?¸¸Íøð?'õ8Ñ­²*?Ó4Մ×?Â?¡+«,ù#?Å-½°¸ù?¶AÃ÷׋™?żÕÂÙr¼?½Ä,ӃÜ?åE[I&år?Ãf¨`Q?Ñ2‰ô¤Æã?ÅVEÒB?ÈÈ~-Zé?ÃgÒ­ƒÔ?á4›zð63?È15¢NI?Ö(Z⤥f?²Ñfp•?ËYpmÀÁ?±^Ø¸ê?Ü*ìæ{R9?²¬sS†PA?Ô½ß9|?¨
å/²¤?ÅVC1ò°%?¤œçŗé?àK–ý̹?¬EÞ(YGMIXED4FGL J1715.3-3832¿ïp3X¿V9¿ªl^Íë±À8ƒ~Ù#ó$À9¤*ëf@£#âqŽ@O	zÓõ?Òµf~ºC?Öa¨üãëÍ@!µÇ͉‹@G+ù4ä¿Â?$ÃÍÕ?翞æàtI¿å^*Ýúº¿èYP¤«›¿ë¡›%ŠÔ¿ïê­R´ûOTHERunk1RXS J171538.1-383531?ˆA}ßåêf?‹«|eÄ9‡?†ó"÷CNü?'Ñ#³ú?ïC+´la[?›¢™ÛNhð?©T}Í䎅?¯ÃqX'¯?¶€Có]?±à¨ÅÞ%x?뚯¿Üà|?¸Š®Ý2'?Á°@z ?©d–SØ´?À–»"|_ˆ?¨áGQOb?ç"å
Âaö?°×g2"ÃÎ?'¿6\-?z²'BVÂ%?¤ô"Å/}$?‰Ò˜é?î"ÄÂ&Å?´CáM¯®?Œ—â²N?±!_
f!?†£t†1)e?.òb±Æ¤?ï5oѧ°'?±»r–Ò=E?›BÕ~5ë? i*F<´Ã?½ŸÊ‹)u?»ÝuQè?ëqðÈ'2?¼=ÜÞ¬?¶Èê'#ã? V ÍIÝ4?Á¸b3É'ž?¨›•rB'¢?èÏ.UË0?­w¾²×?rNšÎ®"?a@ÂcÏt¨?¥~C{µà?ò·a
ˆ•?îƒ~ŠÓ
Ý?'w•¸¹oxOTHER4FGL J1715.8-4549¿ïA£6YÀdÜ"«%³À:oÅåÀ;o§ÿê9@ZÉ!œ‡á@^ne8hý?ÓÒo##p?ç%  ß^@u‡CUÀ&?ÿgþÏSd×?ïό/MËe¿×ÛÙ°
g¿×ED'»Ü¿êE€½ªšô¿êm[}Ë¿ê…M²:zOOTHERsppSNR G343.0-06.0?¤<>VŸ@o?œiG¢<?µçÂ#?®oËp?ëÿHw4ŒF?³ ¥sˆ?Ò6uö"߬?ÆÑ3\?½]K4±¸t?¹õ®ÃLpq?ã9ž'Y?Ä}
ò?ҝ–‹?°@äDwN!?Ī~¹nv*?©.tìëÎ?ᆕK^Ö®?³1¯²?Ä$lÔX?™¥Nffý•?É?ëâUŽí?£Iéqâà#?ä©;äg/?§VpVؓz?™'_EN¯?‰ì¾´Ð?¸øºlß§?²rV…Æô‰?ì­¹¿²f?´SF«Kwí?ºgtT ú³?¸ÇWJ/GB?Âå³e?c?Á€ýV"U?çù¤œµ‹p?ÂM¬ú'+œ?Â]O#Ý2~?¥£Ã—ƒ£?Æ:Ð]G{?°"Ñú,X-?åÚ%'gñ"?³¾'@×M¿?§U†äæ?ˆ˜ÀUÆ2?Éu2mKÄ?­—QÉ?èD	á™ý1?¯.^=F3JOTHER4FGL J1716.7-2808?âXv$ÁÎ@ú&€IRÀ9M'¿°"˜À;'íû½ñ@­ç"^@Ìã"y§Œ?»ÙÁÎ7?×FW}?pÙ@ªTà,%"@ÜðJUd?íay,;È-¿ßÏÔ¿	•«¿ÜYB'uê¿âÿO™›G¿î3eˆ¿ïòüÂ÷ÆOTHERglc3FGL J1716.6-2812NGC 6316?°žÔz—Ö?§¸®
Ã,Ó?çἩi?Âí3»W?È,ÐêW'?½úa£'ª?ÂS÷Žliá?¬˜¾—?ák"<|L?È·C·(1?Ô³-PÒx?Ä
ß.×·j?ÆñÂO›HÆ?®Â"¹&–‡?äaÆ\×W¦?³!lj˜¤å?LJ$=X ?«8`_4o©?Úo{»r ?¢å	¢ž®Š?Ñ@ÆšéG? Ðû&Ù1?ÔO¾Ó©¤˜?Ÿ¿7B# ?¥Iϵh	Ý?™é"s{ ?é6×:[?¼‡€gny/?Ƙ³ËI?¹ýŸH?±u´õnW?·Höp¸Žw?â˜ô«ì‹?ÊÏOÞå~?Öp©kÛ2?ɼG¢²?µ¡.öMÿ±?¥pÉ?ç§ó£j¹?²£0äpÐ?Ə™÷ž˜Ã?®Éõñ£	Ê?Æ˝®?š=ðµçu?ؑþò±/Z?«wµ¹ÍÑ?Ü2ŒwÐ¥?ª‡L}±@MIXED4FGL J1716.8+4310?ç¦}"¼@Au¥ 8LÀ:¿,;È-+À<€g€AÙ¿@l[…íõ@¥Ÿ<pÊ?Ò Š#¯Ý~?àȶd«{@¤ò®å¨@ñ`°D
¿ìõ¶ÀÆÚ¿Ý c¸6<Ó¿äBej½ãü¿æXh¬'Ãâ¿ïÿ½OG"?ìf³ÞiW]OTHERglcNGC 6341?ïG
MEƒ?†òûƒÆ(?ÞGò#Ô?tsÓQ@M?ŽM‰-BM?'V0¤ÿ?íþ,·Cé?«¥S€‡? X*õèS?¢ÛßÑmc?ŸŠ€¬B?˜3°X»á?í\÷Á†â?¢:™ŽCë‹?£~É2ß1q?•[ü§œ@Ý?«ûgQäGj?˜=è¶Ü?îDB­­?ŒžäÃIÒm?™Ô—¶.i?³±I1?¡dOÝNTk?6‡÷;Ón?îE3©"}?œ
´ž'·€?—å!úž?Ž͓ü^¦? &Ú0ùÍ*?"CB—ݵ?ê$DIþH<?Ãs-(?¹Ò|¬^»?À$Ôíúç4?µa¨;æ?¬VZ¨ã¦"?êÌ&æ™?«Ÿÿœ$ZË?®0Lä_:£?ž¡›;rVf?º†¢_՗e?¤T†Š¶6d?ê¢n@"3˜?¨ôUÈw?¯~=Qe?n†ªÛ^¬?»+ÎÝ?®
? »¶4£‰AGN4FGL J1718.0-3726¿á#îaœýý?ÄÅąU"ÝÀ7}5¨Xy>À:*ôàM/@ Œáºö·@Ϊ¦1?©šÂÓ=™?¯J+Ú#@¶w¦)ÊÕ?ûѺyãò?îÀ]ÔÏ¿Ø`Sý®(¿ÞÛ¦d-Q¿ãOl-Îo¿åGÞeü^¿ãÿíPÐÓOTHERsnr3FGL J1718.0-3726SNR G349.7+00.2?•@`¬ãÚM?%b3R?B` õE¡?™±•¦ÕHE?îØóxL×?Ÿ"{rg%©?•ê§9{‡ò?¡D…4ð"?Ãú´‹ý?»—DTÄ?êR%XÌlL?¼Ž¨åiž?§î‰äv¶?›ìR>µI-?©AH}Oê'?rDžžã?ìí
q=
?¥þvÄ{œ?¬ÁpØm/|?Œ
úɤ2?¿È܁{w?›	åÛ?ê:Íbbºy?Ÿ·–"¼<Ý?—c¡'I°s?ŠôpÍ°h?Œý:vö
ò?‰'(0ê'?îÐî
ÚQ?•þNéÚë?'3ÿÎç5?•Pr;å<
?Á!ųº?À57‰?ë0åïL1?ÀVkÔ?¨»…hêb%?—þèüùÓP?©è"0£LP? 1çdÅÕÌ?ìÕ¿fK¨9?¥5ßB³ž?"–š]O@¤?{ŒmŸbl?ÃنÄÌ>?¤=Z~{°û?êlé|Î;?¥0iʆOTHER4FGL J1718.3-4445¿Ì'–NFÆÀ]'@.Ä9À9°"6[àÀ:áJß!c'@ …úUq!@ºizíÜè?Ñ3éܨ#?¿«ó¹J¹ã?÷rï
å?ÿ_Ñâ5iÄ¿ÒC¨ý?ï!ÿ¯"B¿ç%ƒ—×ø¿ãV;`~Dÿ¿ëÑ4Û©ßb¿ÛŽã»{ÂOTHERsppSNR G343.0-06.0?Ù{¯5.­_?ÅnãB¸•?¤Ž0§4.R? ç[À?áùEZõfk?žë§r9?ݗ¹ä¬B?ÅÃ/X÷׬?óFÙå+l?Xªã"Nx?àDˆ×:Ë?ÄÁÍ2€äJ?Ö¦/|'Ã?´O8~Iþ?±ÁS	üÓÝ?žÈSœ…D?âtԇp"?µ8M¶?Ó\qDP´?£$¢®"ô?±6¦òQÿm?Æ9X	?ä*ò"Ê'x?£Ë–‡d?ÏÁîëcCz?¿¤l¤vŸø?¬5ÈÜÆ·?£æl-–4a?æL'·eB¶?ÁSó…
›?È7ïŸN~,?¿ T´7T«?ªbñ™ŽE£?²}ð..o2?èKÔþ…½«?ÀÈu‡
k?Éû›q\?¬½ÝÛ7Õ¢?±¡/Vñ«?žòàc«Á§?燛.3?±`WrßnÜ?½	¨úyr!?›e6÷Ÿœ?´W¦#‰î?Ÿ›ÊGø—J?éÓÖދo?£H¾·j¢ÒOTHER4FGL J1719.2-2943¿×1ï¨ç6Ó@}¿Î·ˆ˜À9Ú¨ÎÀÂÓÀ;(ÇAr'@ !f'jþÒ@¥BDH.?ÂXIؑ&.?¥Ä`A´*j?Ø»›!."þ?ö"±ší+½¿î¸G¿²2?麗*¿ÂypÚ2»ê¿æhÓ]à…ç¿êèûlˆÍ?кѢŸ|³OTHERsppSNR G356.2+04.5?ÜÛ
͹[×?Åڦ֐g?'¢vAb¼\?ˆv·Æc#?áfçj²Ñ?Æ;ÕpV̍?â]fBT8f?Äü±	*~·?¥?bµd¢Ø?¢Z´BǍ¹?؝G%Oè?ᆓ钑?à·Â盰?²‰Æö¯ü?«´'fÐå?™aA}<°y?Ûéã*~¦?±ü¢[í¹?ݔ*vÁ—?¬ƒÉPPr?§ñÝî×:n?Ž'Ñ>Ö?ßmš?åPÛ?«òÅF%K?Í«ýì¡Ëº?Àh6,.S?¥ûÿ
ÿ»Ì? Ev&®Þ?ç5@"Òå?ÁæŸî%?ÒñTóïÕ?Äztù"ÄS?±Ê.ãg½?²ý¶(—Ë?äN©°þ?ÄX»ò£ºÊ?Ôª–hÚ‰?°sucF…Ò?³VŒÞÞß? €ª?ã?ã/dǀ?°C68/Î"?Ìæ¶P•Þ?«²VÔÍø?±D+ÎÆê8?  ;³Û?æÍw€b?¯6ÓR'@ÓMIXED4FGL J1719.5-3858c¿ïì;gŠ'â¿îýÕôéLÀ96^q¥^ÊÀ:‹™¯i·@€‹Ò† @Õë#Ïèá?Í:†ä‹/t?ÓÄ7Kæ@tËáëB?üû]y,畿ïÔY=ÞÝÆ?ïߘa5O¿âÀŸAú m¿êD
û¿ïú}¢Ã¿în¸å;rOTHERunkNVSS J172006-385734=?Áö"(Õûä?¸«¯Çö|³?¼æyù–?³þuÄÛÅ?è>r›AÔ?À~ÃùÙ91?ÀßC$ {ê?»X‰ë<?ÁX;©,^?²ëÎdJ¡?çr LŒÜ®?¼KÎ?È©©É´áÁ?«ôM(ّL?ÄH€³Úè?¬•³–Qÿ?äÃu`²ÐÖ?²Pb&Ó?±Ý1Z&M?|"®ýŽI?ÁŸ"óV=?œJZ8¨	–?é‡Üt×å§?¢CÒ rè?´"±E«Ýs?¨æ*ì½­ö?·Yޏ4>`?±¬í4¾|?ê".ye?¸›Nôôwû?¦dE'fI?¥ŠuŽrU$?ÂÝ=µd±?¿Úü#I?éâl@gpŸ?¿¶ù¼D€?¸ÊÅèU_?Š¯K%¥þ?ÂG'.få?«ÍTÜ 2î?èTÂ÷®DC?¯Ç£=î^S?—ÿ" 5•?Ëfè6˜?ÂHºE®}?§å'&:›??ê±Ñr46$?¨Û§ï¾VwOTHER4FGL J1719.7-4500¿ÒM™ƒý® ÀÃkL4"À9°üQõ–À;¥5¯v@H·"ª—C@Ók'/É?ÎÙ6´Þ?Å°"UÕJ?þ*Óé À@#T²^âd¿ËP§!íeŸ?ïüFlÊ¿è2æ§ieõ¿áȬar`Æ¿êv?A´U]¿ïՓWPOTHERsppSNR G343.0-06.0?Ý0~ärÁû?ÆîúQÈÓ?¥+ªCSõ?YR#/ÒM?à"ëp?ÅÜFÿæ!)?á(øן!?Â5œsW]?™EJ"U9?"þ6Vr5N?ܹ¨5qZ?ÁrŠi®x?ÞØOÍGÆé?´Ë›*Ÿ'?°Ùq4-€­?Mò93v|?ÜñSæmC?´m~l?Þo›´&Ú?§Y×|r$1?°­d?Î*?ŠØF• µ?Ýe!sSoû?§'iR֜?ÔùR'Û²?À_}^O––?¯ñõ»®le?¥ˆÞWl?ã"7[A?ÁBƒþQÕ
?Ð
Îí…ÌU?ÂFÓ'A?¦‹|â‰	š?«Wà ù'?æ'àºëMì?Âð`|äÏo?Ñx¾Òë?°è‹¿ó<Ò?¶€Uà87Ë?¢§AÆâd?äsëäXôR?³G×kGˆ?ÎêÅ»ám?¨$bºF°?·œS¬Q6'?šƒ/É'?åQÄ´w¨?ªÊÎt0˜=MIXED4FGL J1720.2-4757¿Ü"jÈÏ_ÀÀÓI¾óÀ:'˜Ë=À;K§ågÎ@¤àDMâ·@¡/ÅÀi?Þ³ÞY<1?âéà¾ò·@	å'^éšc@ۚÅ都?îÁr'¿ãF¦ã.8"¿êí¦â'Q¿è"s?ã­¿î±CD"o¿ï¤rØœOTHERsppSNR G343.0-06.0?æªè"‡¹?Ã	û²Ï†Í?½ôþˆöM?¶
8©v?ÆÊã0Ä÷t?½81V0±?Þªy"óE?Æš	šÍ:?²:ŽíÕAL?®1­0½?ÜÆⰗjž?ÃìK\
¶¼?ã{ƒ·©?²
¯¨Ç|?¼éL°;>?§0)²c¼?ѦµØ$ÕÞ?¯¸Ù¢²?Õ-C{f
?¥¦¸¦¥?ÈvD}»ö?§hwÌ`"?ޗšE»öç?¨Jí¥i½?Úü]\Òi?ÃæàQíf(?г&N"ƒ™?ÃþÐÉYé?ÔPÕT©þ?ÃOGE¹É?ÇÔ®á‡øe?š]±-e?Æp÷Š¡À@?ŒNÛõ?än–dõ'×?Ǻ:,»?ÙÀm"Ã#?´¢$2EiÅ?ÇÚ 2?±#ÚTê?Ú¼%Ó¬Ãv?´î´ìí?º\ú4—"å?Z¶ ^±q?Ími‰uMú?º¢Ëw}?åYW¹å?¹š:òLì MIXED4FGL J1720.6-3706?ƒ³(xÒÌ¿°¸XÌtã,À8§?LF)°À:1²þÅm]@>w|ŽEþ@S½Ö.u?ǚÕChài?Ø ê@%@6Vîú??ô–óT Å?énÑnòý¿Ü.®¿²‰¿á½I6ª¶ø¿èÚå>]³º¿ïÿðEwÙU?ØddIU´OTHERunk1FGL J1720.7-3707c1RXS J172051.9-371033?¥K{²©Á?©À€}Ý´"?ÀB¨Ï ?¢¬ˆ̈́?êŠ÷š«½^?Ä´
a)Õ?³ZÒäõÕ³?²¢Â£ƒFT?ÈyòG¹/À?»ióÊùl?çv)œ4©?»IN}'{=?ÁD¼²ù<?¯-\þŠic?É)+÷P%?±hÞN2¸?åd†ÍMP?µ¼|*Ýt?‹@6 ?p[÷>l?ÄÊI`'\ø?¡!mpÆj?ê`mS¤þ?¢_]Ľp?'îç¾eŒê?'ý®ò_@?ÄK…hÎåE?ÁJsÒÆÈ?êU§gô—'?ÄwÏý%Q–?–÷¤øفL?œÃ¨<ÈÓÜ?ÇÓ²_½]?À01Ԗù4?éSVT܌o?À>Mè$—?µGÞú)"ç?¢c"~ÎõÃ?Ì>˜…â?¶UÕ'Aëæ?æVôzTž­?¸QGÚÛ?h&¤>m?T:àQMÁ?Ç·ø<Ŷ·?«xNL<@?éùÛc='?«ÂÀÉ"7&OTHER4FGL J1720.6-5144?݁¦~À ¹y[5°¼À:¦úX÷À<"hê¥$è@ ²šl'p‡?ý	¨ÛUüŒ?ÐŒ¢:R?ÐÜ¡'N?ÿàjْ­í?ÿøwWû>¥¿Ý¼âÉä:¿ïÿÍ?¹Ss?ïÿþøþ"¿ÂÜËG'	¿ç+ÔÏЍL¿å»¶ŸŽÑOTHERunk1RXS J172032.0-514414?íIGÊÍvÉ?ª¸í"pÿ?cyÖo]¼ç?UlR8[À?µòõâb?ª}h
«T­?éž(
Ü?Àr£z\×5?rªåyõm?xü-Û?Èòx5¤ZE?À"ó9–?ìOŠSqZ?¤k	IþÒ?"÷nŽ	?y«‹5 ø?»Q.ym²¿?£ìg,1R?ëÂsZž:?œí´>"¡Å?€?ïš/SC?n3Åu˜C?¿çærI?œ›RAÆgç?êF¿d"cý?¹C{è	½?s³ìb–?iZDÒ¿kj?ÆGc
bán?¸ÿ#füF?ãT³›*?Ètf˜?€3Å'¢™?'—êRºœ?ØÖJpLÕW?ÇÊé¢	nƒ?è'"º>?°9NfA?"Cϖ}F?‰40_ùwÁ?ÍEU'·/à?®ë¢{Œ)?ç'{7™†?°èË@f¿«?ŠvoÓ4‹q?‡jXÅ[AÚ?ÐV€À.Ú?°ÍéŽÙµAGN4FGL J1720.7-4629¿ï£='¹éÀºÆü©3kÀ9«;_QŸ/À;蚈¬â@,Z¢7øÀ@
=f?Ò&Mà]£?Ú
™¶õÊó@ýÌI?ü…jpUÊ¿àŸÖ"Ì«??ïø m]Ñl¿ë<7ž|ØC¿ïg6¥®zÒ¿ï¦J'Qž?'rs\e~OTHERsppSNR G343.0-06.0?åU"-bÓy?Êñ3<1M?¿] œç?sÏ+¯Q?ÔHáˌ…à?ÊX­šqI³?Ú­Ù¼´s?Ɣ©MtZ£?¸Ÿj">¶?²ÄUŒîæ?ß*e\ƒÂ?ÅpT7 ?áÄã­Êå?´X ;8)?µ×¡fªt?¡Òsãy"?×QœÞP6?³9:oxÄô?ÖG¸:ïj1?©˜ˆêC:?Æ™ÇD€@?¢Ëwí_Z?Þ©úà[tñ?¬Ï&‡<ð'?Þb·òö?Ìp–ÍÙ´‰?›£íû"?••ÿÞ@>?ßã¬v¯Î~?Ì_êûzÎí?Åڎîè"
?Â"S×Ì?ŋs?Žû?Âùç_þ ã?å&te"¿?Éþ‡Á<?Ö¬7B®È¢?µ»8ulˆ?¼}'‰ÒH¯?¤É%!j§?á2
nR™?·T¥Üüxj?ÁJ™1Ðî¬? þã8ZK?ˎxJ¶Ôà?±Âͅßq?äÉ» Þ?³=¿ÍàÉMIXED4FGL J1721.7-4709¿î‰Gj*sÐÀºeÏg±ÀÀ:Ɨÿe¦À;œèÔjP@£©blD@¥ýfȌ?Í喝:ã×?Ò@$]Wt@,^b‹æS?þ-
gbé?åùæuë>¨?×|Š_iòã?ìÁ֙Õ(¼¿æ˱ÿÁ쟿ޒñì7Ì¿ïþŸã_¶IOTHERsppSNR G343.0-06.0?ÔZ›è?¿´‹مÝ?€o×MŒ)^?r?A~?岺udä?À—_W©_?äfú*SÇ?Åõ›=Ö?‰÷ï8¨*;?p"ìF6\?ÖbL1B(€?Än€€å;?âËÔÄå?²RM£â?¨t9p‹™¬?•<³a,E?×YÏJ'¯Ñ?²`ßF?ä(²ÙËì?µ<2:ƒÂ?rXHQº?Œ#䒏"Û?ÕÜôÈ>r¬?´î"™M?ȝÕÚ£¶?ºën°YF?Â«¿>¢[?'ºðZáB?éa®[G¤Y?»¢L¨q›?ئ¾÷ˆHu?Çûo¦ÅÀÙ?—^^æ?¤ôY"¹Â?âñ¬y+v7?Çw4Áõû'?ÖÁ#jy'?´ùÑå"×´?±eÇÅéé?›c©V‡?âr¿õ›DŒ?µðöçÚB¢?ÚòÈtxwá?¾mš=¶? ÷÷¨*œ…? R".r8•?áwK\—'?À=}i'üMIXED4FGL J1722.6-4529¿Ùl3¼½W†À…³ž'ÔÀ9¯Ëú>õßÀ;²Lþ
@ÝS­§@ì``'çÏ?À9yþ§?ÔØVB×Àò@'j¡^‰ù@kn|Šj'?ïµïpeé¿ä±¢Íõ¿ß
J 4¨Ô¿ã‡#uP5¿ë©ÿBjß¿ïúêû‹ýOTHERspp3FGL J1722.9-4529SNR G343.0-06.0?Ì2!'nNŠ?·_Ôk|8?Û®Õߛ?€wr±?Ö8×`é=¶?¾SÀ1
»?ß­¡î?Ä+9óxÅ?²à	®i/P?§N½Š1@?Ü<PŒÌN?³Œ¼<?ÛJÙª€È?µ)çZ"ÀK?әä]J'?± n™‡9?ÑþÉI4§?­2ʉyÜ}?ãñ<ؚث?œîÎ@,…?¸dÓ§ºø?Š?aÿIWÕ?Ò…Yà_ë?šAwÞLÀ½?»jÀEÞd-?­.•ØƒŠ?ÞaÇ+‰Vç?ÃP¢И<?ÚÈÄðÌ?ÁÕë¼H'?Îj{ôÃ?ÂÇnÒº?¾<)üÓ¦?·d«K‰?份ÛÃ4É?ÅõõÙ4Ä?Ïfíæ™?³'ΗÇ?Ûs…[§¤'?¸«"{1*™?ÔÙx­Ìè?²ç"Ùƒlñ?Õ°¦þð?¢(MõtP?ÅC¹Ñ{ô?žÖq–d>?ß®pDX?¥Ò³çY³MIXED4FGL J1725.1-3408?øΊbð?ë2~žºÀ8ß\Q9®wÀ:I‹N};•@N.4ñ¤H@îu5¬?ÉNÚX¦Š?¸Í®ôõ‹?óü8Dêëœ?ü§5Ù«­m?ãØ'>2j¶¿Ú»k{y"¿çRª&¯—2¿åjþ¦Ž ¿ì¶ ¸Ý,¿Ø/EâOTHERunkNVSS J172445-341032?"`EU˜»?‰"ùÑ©»?"ØÒÚüçý?ƒQk3&s? YZ?'ßÌQÿ[}?¼Fí$[)?¼MÀgn?¤1÷>¨kË?¢K†…"º?ë4çn—@?¾¿c,Ë2?¾ÞúCIù?¤}HxfY€?´Ñ;³&¶ã?¡ü¡Rè?é‰ùA[%Q?ªÊ±Òfü?¼×®h€?›	ËBρŠ?¡m²Ã³´Ó?€*¹•wö?ëW	ï—ýã?Ÿgכ+ã?ŽU‡ÿ©ž?˜üŸ#ƒ?yIÌ®˜$?t"` £Öä?ïT,`tú?‡´£ŸÒ¤Å?¬'¡œ¬ÐV?©˜ç%áf?¥úEÄ"¸?¬øYȒ8N?ìÝáŽ,??´iq5ˆ‰?·ŒÇ£=w?  i¸ó?±æµfŠÀ¼? ,]xx"?êѐ^Ú?§ç&ZÖ¼ð?¢þréÚä8?Š)°ð¦°S?¢«?àõáŠ?ˆàüö~š?í¥dÓ`²?•N«¥ØOTHER4FGL J1726.0-2843?îÝ(Έí@
çTm?žÀ9ö·ü[/ÑÀ;Mx2@Äì@ Óc®ün@7‹7GN?Åa°ÊÓù?…³sy8>û?ÆZgª‰+?ü{Ã	ÕkØ?ïNj׆¿âÁž€‰'\¿ç	ýڶſåf:âT¿Ö¯šâÄÜ¿ãyÔ½\OTHERspp3FGL J1725.1-2832SNR G358.0+03.8?ÛÙ?½ÁRV?¾ý£Œë?c|EÞùûz?U'yT(Åø?áÿãÛ1>'?ÂÆ:ùómî?ãâ!6Ί?È+=µ1?"»TC=?—-d=÷oS?Öû1ގ/?Ç|vúnÏ?ä
]³SBâ?±t—Á"*¿?©ˆYhA¬?²'ʬß?Öà¬U¢?±JvCCÅ©?ä
'¾5o?¨#®áŠë?ˆh¯¨
ù?pcX«™÷?×"kU¦ó?¨0BÀ~f·?̤zHE"?¼cˆ"ÓP
?pªr°ÒÀ_?gø¹)Y?èÝÁûý*Ò?¼ªŠ®ï?ÖD7^ÆÆ?Åöÿ{­?˜5áÎóù?¢½¡›ý"C?ä6TOãm?Å¿ðÂÓØ?×ຄ9¥?³¦Æ0"	î?š" ²Ú?‡NÎÒÝôB?ã 3	Óχ?³æDà€?ÔÁ[Ø¡tã?°[àl
?"'ß·ÀÃ?† wj€ã{?äú»ÏY?°©okp)MIXED4FGL J1727.0-3835¿Þý6¡~¿ÿóÐFÕÀ9á¿uÌ4÷À;ác\ƪ@ëE	¬§@a/	ØÆÖ?ØY<k?éÇE8ï4×@
ÜT^üå™@'Ö†ßÙ¿ÂXG"©¿Ùn<‰J"¿åî'Z·Ü{¿î‰¢«'¿Ô×Q?ãšÅ¿ïÿs³VBOTHERsppSNR G350.0-02.0?ÌÊ"î—wÖ?Äáãx"?"LO°pŽ?ƒWÌê"Ú?è|G#U¸?Ä̪½Fê?ã͒uõ
ë?ƖÊåÊ}E?¥êD]Ñ7?"hhÄñ?×Z|o´7?Å¿øåÓ]?á^4±7š÷?²Ö9_¬"Ç?¸ð4ípÑç?¤ì7€‡ÀL?׉bPx?±ãiEŽ¶"?àË'~>?¾2/8c?‰¤Œ÷%º?z^;qà‹?ݜŒ›·ßˆ?¾Ì§Öü¯?¼p©5mõý?¸=ä"Qó?ˆ ÒEx(\?ˆÐãÓf©?ìg ã¿?¹Äïàá?Җšýƒ	F?ƼV%õø?".½˜§?¦vã˜2"¼?åȑUž˜?Æóçè?ØŕöÌÐ?²ÿÿ"V[?¾	²¤`$¶?¨´Twé?à8fàx•?³!ÕÏÜ ?ÒÛN•'Æ?À囡lÝà?mݤ?†éc½ým?æëH
	ÿ?Á"YyÒMIXED4FGL J1727.6-3050¿Ñmk£g"Ï@@€"ÐÀ9¼'xêÍiÀ;<Zݜ'é@/§x#@ŸìÝ
Œ°?Ç~÷?×q,½ùf@	C¦GýÆ@kóā¿ï·âÅ\–?ïøÙ?Ìɝ¿ÄðÂuZõð¿åZOÈl–¿ê} >ÏH¨¿æû¼Ú'.OTHERglcTerzan 2?ÄvÅ}¼Þ?¸Ãˆ?'Ä?ªZìü]û? ÆZXÚð?é<ŸÐë??¼©]±áäâ?Í}™Ëe?¿õ†2RÁ?Èüß­,Ñù?À·wsC?âaa¡Û‡{?‹Hn¿âj?Õ5™Èq&?¯¾Í÷îYR?Áµ\yµ?¥u–Ë' ¶?á#›÷©?±C-#R)=?Óûjéq·í?¡äQ÷å?ÂHÑލ;?˜TÙ	ìÉà?áp£Üû?£ƒšôæX?±#wûÐu˜?¢ˆñY~?´,ðô«U\?¬ú!ÆX§R?ëUòáð†¢?³wÔì¹£¼?¸u̝Ãn?´BO©ã?Ñîpw¨>?ÇNZvC(I?ãú0fǂ?ÇYÆK´M?ÃËÌÔ{å ?¦³B™øÓ?ÅUIw\?­ršqàÀ?åÌ÷xƒ/±?²jOï o?À§‰HH?™Oß¹n[?ÇïjFê¸?¨ÖÐExO?åÚ`s@?«¤©Ñi!OTHER4FGL J1728.0-4606¿ØŒ5˜hA2À
çO/<À97cf×¥nÀ;-±@óL/Çn@¿Ue""?¶¯ÀøXA?Ò>¨\U†@"q VL=?ø3
ÎʨÛ?ïÿÙ¿y}¿ß$Ěúݿ჆g­Ó¿æ¥ÒWPHî¿î¸Ÿƒ¾f¿ï÷q†U7OTHERspp3FGL J1728.0-4606SNR G343.0-06.0?«GjY²pM?£ÙÈp¸?½"ïÝ.U?¸[ó"'8Œ?ê™_Ɖ?»Á‡×ґ?±}Ï5¶.ö?³Àv8»å?â|efa2ö?ÄØÁd—?Ö§Áe¤8?¦ï|"é?Ì´ãÛöÐ?¯N1Ïvn?Û£ ‡?´è!‰H±?Öþüä†l?±ˆ¼i·°"?óàUq^?–8Ê+DÃ?Ýóžf÷Ÿ£?¦ƒê¨!i?Ø2qoŒˆm?¥­Ilä?—å?~RèÇ?u"›vë#?Ë·½þË?Ãytú¸î?èR愃ÝÆ?ÃÖ­1'?¾Ô¤v?¡Âbt
ª?ãýJ}Ÿ	'?É<Ô<ãÛ?Ö)'3»24?ÈúØ>×…?¼Ñžü¸€?¦Ðd/J2Ž?àYš:©I:?¹øñC	ü?Øgd *?·p!Úï?ªH¹mÖd?‡ẉm?á8Dêì?°ÏɄjsÁ?Ú~Ç£'?°'=^§¢"MIXED4FGL J1729.2-3641c?ï
}¾"¿ôŸ(NÓ£À8Q•p?-<À:LÁ¬Zg@·
Rê2¹@ríãÉª?¿z—˹&}?Àp£$è@SÍÅ@Ñwò)þ?ïà!sNÑ¿áˆ8õë¿ákz¢]z¿éOJ@ì¿âŒÍ}÷§—¿ë	—"ÆÔeOTHERunk1FGL J1729.1-3641cNVSS J172917-364008$?Óñ¤
?Á­x.öô¥?Ÿ¤õ·4†±? ¾&vúA×?å
NН'Ì?Áùÿ=•ëB?Ïß7­IU?Ä3é]ôtS?©H÷cÐê&?£™º
YH'?æs¢ž[è?Ä1îúôþD?Æ?‹á9?­è¬ßîÿ?ÂõC£î²%?®÷™ ¼Û?å²èt6?´%Ûçá?Ämº2ôÓ?œå"o4?°¹6+Bö`?Ž·¨ª,?è͑Œk? ä@#Œi?ÇîûofY?·36%Ódœ?£ÿðé÷%?¢ëF´•)?èÓÁ%NÄ?ºÎ×~8?¹É€]/?·'ú?²3¿ÈàâŒ?´Ú°—
i?ê€dö"‰y?½nÒµ]ß?¿W€áV6?¦r"ÒG{Ž?ĆlÁmÔ?²kv/W§?æótËü9Ä?µbžV}÷8?©pMïòÍ°?Œ½‡Ðèg?µ7÷cy?œå
ž/$?ëÈT!ë7F?¡(ÏLÆèOTHER4FGL J1729.9-2403¿äßÖâá@@]•ÝLwÀ9s†öÿ¦À;)½¥œà@̏›"ï·@ìB 6m?È{™=´?â}
!P² @"‰|ëãé?þéÁ¢w8Ç?ïü×÷£:,¿ÔÌÕUc¿ã¤¡Ý5¿ëÿ‰b"ʨ¿ïõê28ap¿ïù)¢ßÇOTHERunk3FGL J1729.7-24081RXS J173013.1-240234?¯-å+}[?¬¶Ü|?âµ'¥®?̏WšàZb?×äØUÛÃz?É ÛQØ?¸#¢h®?ºÈRÐÎ?âEZä8_~?Æ2µ3þà?Õla–âžà?Õem˓?Ë(E¯ô?­:¸'Í?Û˃å/øŸ?³/\š×²?Ö pÀ&?°åælc´
?¬ÿÅ$eN´?ƒÚ¢'¦šÛ?Ù(ܟ†K?¨ÿÛ2K?á›û¿\)?©'";â?—ëªCÇ[?'̓DÝC?âü¨ÿVü€?Çíüøu?؇ó]ŸZ?Æi¡.cj³?¡ï=èmè?«¤«I$?äi?sú?Ê([éµ»¹?Ôðyå@®?ÈÙCë3·Š?½®ÔO‰?¥±'Ì?ßäN:Âëð?¸#ühk°E?ØÖìˆ.?µ4ԉÌË_?ŽíŽð:"Ž?pg(-©?ÚÛ§ýE̤?³c0[Ow†?âuÅ©íÐ?³tñ#Ü7«MIXED4FGL J1730.1-3422¿Ë£ë+²‹¿ÂGUêmFªÀ8¦Žt¢À9šÍÔ3É[@¡Ìzd@½Ofo ¢?ÍØ&ݏg¼?Õëòa±ËÀ@'؈v\?ö¨Z†¬Ø¿Ü«®¤Ã™G?ﬥDȆí¿åހ¾×@Ä¿éclK'µR¿íT¿	•ªø?"Ö9`°*OTHERunkNVSS J173013-342115?…¦ÝA<Ÿé?ˆîaãmúº?hT®˜XJË?oPÿŒëâ?ï'Ü/Úþ?*©õýà¥?°X!ýqS?°µ"f?ÐǀÌ\ÿ?¼·/µ,û"?åè˜" Ð?½Èoš™t?½WυõÞû?¨$sHiSÀ?Âa°¿Pˆ?¬7ܳqGp?缙ßm@ÿ?²Gº
ÌT)?ˆé՗Öó?s
W>¤¯8?Á€ž9Ö)\?£·~#œg?ë<1€äí?¥%… "]ë?rB-™ºªw?v¾,!<?yÿßP_w?ˆµß
Ôõ?ï©Q¥ªÜ?Œðߦ?"Y¶L$=C?˜Fä]:­?Ô\ԟ?ÅžqÖÃ,?å/,c
f`?ÄÆëZñ,?³ª`ÁT×?Ÿ
ßmŒ–?ÄVٚTn[?¯ä£ËO2é?èv"LäÆO?²Ë¾œí½Ü?k?v­e ?ZÓ½"?Å*Þ"Æ»?±¹@¯ÆÍ?êš8Ñ`bõ?±:ÜY²¤OTHER4FGL J1731.2-3234¿îdz§'?å$Ðd1À8yÃ
0j+À:?–fß2*@`¿ÞQÚ@,€"Þ?¿^•–Ö?ÓhOŸ¥wH@»4¾?ù@w?ïÂ*|«LJ¿Ö"¦%=d¿àã7r]¿ãÕ¡Qô¿Z¿íoJpfši¿ïÿ¸aÛ½+OTHERspp2FGL J1731.6-3234cSNR G355.4+00.7?r¦ÐKÍ×æ?qè=#˃ñ?ÂÖ9ìúƒƒ?»óÍP2?ë%#ä>a?¼DâÞ0?žæ·q«Dæ?¤9*ÀH?Ë¥ØâYÑØ?ºÀbõÝV!?èTÎró?½"wú@+?°ÏV¹Ññš?Üú'µ÷?Øv.°lš?²»èBýí?áÛÚ6'À?²|ðþÅo?ZÇV(F>?q'œ×¢x?ÃA\I_£?£&å´.®/?êº=Ð3ùF?¤Wè¥>•?yçëGu"?u`{×?Ó{B|¸s‹?Ãi±¬WXÏ?æŽë³X?Áà˜]?ˆ"\¨Ghg?žª®'?ËWu6&ÇY?Àð]¯¢^S?èÇÕ?ž6È?ÀïKJðÙ?¤'›¶‹_?"¯º¬
v?ÛÌçÙ\l?¹ûõn×y#?àÑbWÛUž?¹¯¨õc6?osÈ*¥í?ZåÇÿúG?ƌñö'7?¯|
Éyß?ê=Pm€¶õ?¯yÀƒØUOTHER4FGL J1731.7-3445¿²Û\ª_kt¿ãØJ¯P»À9£££Þ–úÀ:ÍÛÌDÑ@!ö]¥øw @mŸ¸—Œ?ÂxžözÆ¿¦ÉÍÂÐ?é÷3]z"@û»!ԑ?¢·µ8†">?è–._äÂ¿è‰ù¥ôò¿ß''%οêNûæ•Ë¯¿†WýS8OTHERsppSNR G353.6-00.7?ÃÒ>¾N&K?»A'©\ҋ?'®ðÏӕÓ?¥Xvû¿;…?ê}øÊ	Vž?½1,a¡Ÿf?¼L§Ÿ'i?Àz?Š;€?'¯å²ãã?"«
*"!ð?ëèëÞ­Ad?À3¨è°È?Ó"i±Ÿ?±D²y0åÈ?©ÚäÙ?™°½–†¼3?ä®ý`aC?²ãuϝ´?Ó¼Êîr±?©b€À¿)?"Ä"Gà|?}'å.'7ž?åx|úF?©6,Э&ö?ÀÀw
'½?¹'â
[w?I© ³l?†Âœ¸¬6?ëM"ó"õ?ºzz*Ϟ?³]jMØyI?³"%^S%?9REÂãÝ?ý˸ɷ?ímm©ø?´•ë
†z?Ç´ÙÕ¸…?©Ôؗ­Ç~?¨£f«hu¡?—Ñ@õŸœ?舓éµ?­3—eš‹?¿´å
Âaö?£Ø)t´$?šžÆü"•Ã?
¯‰Ú…?ë4m&ìJc?¥Ù'ƒÕÖïOTHER4FGL J1732.8-3725?ì¯;íAŽÀCÁð`À9eV2;¼oÀ:ìÍ҆J1@"~'¶Ñ@åH©¼ýL?ÑSÇ'q^?ÏmŽä3ñŸ@ˆÚ¶š[@?¯uxýî¿í$Ò°+¬?ïõ9Ó`dÅ¿èê$@ÒA¿ä—™^á6ç¿éÿD^(Õ6¿çÃlfZ§ìOTHERunk1RXS J173250.4-372144	?âÎÊi_!?ÇM¬TËù?¨P–iÔ? «5%æ>o?×XX`8?Æ{E»Ëó‰?×ÇٝëØ?ÅnàTáP4?°ì@͛÷?®8÷³ÏQ—?áþ‹/ëÍe?ÃrVè!ŀ?×¼=B«¡.?³¡qlÑOî?º"šè+Ö{?¤ÍBBŒ?àݎD:?´"šÙix?ØU›š6o?¤{&z³½l?¾›-ºÅ°›?š{'o]ô?à̈Ú.µ?¥%‹Wqý?Ôð7šù1?Àìܗp¡?µÎHµ‰?ª,¸Þ—ö7?âÎ"jc 6?Â_˜ÈI–ˆ?³[Þ3b¿?ºAùŠ¼?¸ÝE°'L?´¸äúž ?è7€R~Z¬?¿•ZÛé+?Ç2äaq'?§íÖô"Ç?Àª>…̳?©|«(5žà?æÁWx·Í?°v¡R¥³;?Ď´4NÍ?¢
sØ\&?ÄReÁâ?¨Ëu:½áº?åÕ>_Ù{Ô?«ì".-MIXED4FGL J1733.7-4734¿ì )ZHÙÀ@š$À9ô§5jEÀ<Tsõ›@ ÂÄT­×@ÔF=Ñó?´Ÿ&y¿°ÒÖ|#'@Òß5…@h]‡º;?ïûw¾Q4¿àÝe4Ù&¿ë¢=aàDÏ¿¬ø[EöÚ<¿Úìé7fž›¿Ýã_ ÏmçOTHERsnrSNR G343.0-06.0?ìµþ|û±Å?­Fب3v‹?p4s1ø`ÿ?cA"	Õ£?¹LÄ溹Ä?¬Ü%Ü趩?éÒBèÊÀ?¼N<Îè[?k(R|C?q¤'^xn™?ÈJW¥n?» ùl4~?ímÝ!?¡o§kx?€½tMXp(?{mèÀèá?µèœ#F2? É=ÙÑÙV?íöNažÞ?Š‰i"¦è"?}/nLú²¡?cl­{ña…?¬õ,;úÓ?ŠR8kˆ8?èàÄȾÃ?¿´W¾‹t?"_Òù	µA?|=½½r·7?Ϊ½FêB?¾Šá§Ç§?ã5sþ¥e?È»0»8?sHê•lZ?€þbò—¥a?ÙGõŠä¨"?Èx-vŽZT?é‡Ý›?¬b¶Óm#:?'N6ã¥?‹¿Ãæ#~î?ǟ¹ÛÐÃ?ªu~zaùx?éi×ÝL ë?¨ù8•¼£?œ>žq%ÏK?Œ¸L0[ò­?ÆÐ̺òôn?§"›¬-íAGN4FGL J1735.7-3026?ëJ
iø ?ðZ|MXxgÀ9êCÖ¦À;Ô#£s7/@Ã՟.Y@âñíÅï?ȃ§¿Í
?ïÿ¼¾ŒÃ@ÖþqŠ†×?ö39=cc¿ïø⚔k¿ï|˜6Ã
¬?ïÿ÷fÔJp¿ßhóžó ¡¿îÈ3'˜¿ïÿyýò߆OTHERglcTerzan 1?qP©ìȾ?†÷L}1. ?ìIøú}43?Âéži?¼›-‹‡Ý?ÁʞÎ{'a?‹RucÓn?žvyµÌ˸?ä^忞!O?Êæ² •{?Ög ØÓf?ʲ²ú镰?»üR"€Ö?¦aôȱ–?åaEa«c?²X/ô'Î?Ì|Á,ì®P?®VýLM_?†¯{òÙj¯?tô˜Ñ>F?ë'øÝÕfW?´&{$Ì?Áõ$É|Ïù?³PŒ_tYÄ?|–tXéç?¢£Š×u?ì ß|/"?Á£
iR²ˆ?½¥ßžÇ¼ÿ?À÷eßU?wÁ^ûÕ H?ƒOvôŸÂÝ?äõêµôw?Ï)—º-?նʭô֒?Îû…‹´mt?´—ß(pÁÇ?¢%¶JŽË^?æWC9Kâ=?²_àØî€?ÌW‡sý(?°e5ÒA?dN™@-l ?`0´Ò©á?ìMD½…m?¶ì…°?¿!i1?¶ž¸TFœPSR4FGL J1735.9-3342¿ï´<*'Æÿè¼Ý W
ƒÀ:I¡òYNÀ;•ð	÷y@$>ìW¬@?öúReŽÐ?Òõº+àY?¿/øìˆ?昏Bþ'Q@L¨–a«Â¿ÙÝ>‰þq?ìÕ¨]ס'¿ë¶y¿¾ë¿àt¹°V$¿ÚC©blD?¹kt~hLOTHERsppSNR G354.8-00.8?ÅT¸ß/%?ÆU¥TtÉ?Rv‡Êº?V¯(Ukc?ꡖ¿¹W¿?ÆdËÚgÍ?¾¡ÉÕÜÛ?
¨ê3T?ŽÚâ¸g';?•í[ÂÜN™?ë°[UCÜ×?ÂÃxGÂë?à«Ëkª?·:–Ï-ÝÛ?—i+¶¾ÍÄ?(BìT?Ý1×Æ­ñ?·7«i°Ü?à4|UÞP?¸ŒãcMò?ŠD§ÿ×ÉÓ?€'ˆa6žq?ßqÇ:1?¸òÉ-'wá?½æÎý9ã7?¼bÞÔك?l»,|?o`ÈS¶?ì'åý?¼´áÖk©i?µh|"÷b?º£Ö*æÖ?€Tßö?'qqš<¥Ï?í¬0'Ü?ºqrLèT×?ÕL"L?…?³vÄ;/‹F?¢³<¸*ü?—¢	òËxµ?ä.'miK.?³íÂm鶔?Ë¡0‡o?µÛæù§Sõ?ì«û¡?"eÏ[«?è›4+€·K?·Â©õÔ¥VMIXED4FGL J1736.1-2628?áÛ6:	ø@Ž)#øÁÀ9Ë~>Ê@+À;!ë¾íç@8Å]F­@"¨~8ë?Ò.!%"?ގÍbÉÎÁ@z?|ÑÔ?ø@ƹã;#¿ïýV½{öñ?ïþ¤ ³¿5¿è3«=°å'¿æÌü¿ïù÷<âß^¿ïö.$ÖyOTHERunk1RXS J173614.4-262806?Ù}ÔÙ<¥?ÉãxÎÖ?ºüX^CŠÍ?¸	ìE––?ßÃɕà§?ʬF;ðé?È1ä'î8?ÅëȐ}?×ÀXÖìòm?ÇSeØ¡í%?Ü&´à	÷?Åuʜñ½È?Ôã&TlW±?²%(?7™?ÄÝÉM«i?«ãªÎ‹?àVú'_Í?²¢~ã=?ÅÐņBµî?š'"‹æ3Ã?Ô>فà?©0õtÄt¥?à|/2jô?«&ã~A?Ë<²k€4?½ø5J(†÷?ÅMà±cÃR?Á³›–|ŒK?ã鸦'¾¿?Æ:ÖÛ)Ã?°T¼ãÔ-ó?¶CßÅ+?ÞÛ"ܵq?͹ؠ·è?Ý­êUì?Ëâÿù
â0?Ŕrïœìœ?¨l'@%T?ÌËR;>Î?¸KÛÍPX?ãh0e…?¸q'ãÄ?¯9±Aµ?íD@À;?ÖÔ
Ò£ã?²·¢E\"?â¢^vzR#?²ÝXRé?MIXED4FGL J1736.2-4443?ïÿtŽaÀç"~§¥ÌÀ8¶A+Cz©À;›<Õsd|@4ê³èzR@.Oü—•³?®éùOÛ¤?×{z«í¯@%	¼râv@n¦R9³«?ïóÝ£C<¿³3ãu!¿Ü<Î<Ž{®¿åp³[â~æ¿ï ‰bi׊¿ïõ8%á;OTHERglc3FGL J1736.2-4444NGC 6388?8Š‰Q!?'É×$N?ëc¼_cµ?¼ë""X"?Áç_¼tÉ?ºˆÞÝݲ?˜Ð`–rçŒ? >ÄI¼#Â?è:Eíä¹A?½p´`U'?ËüÜ6C«H?¼£ƒNçá?²#x­È?¤LC|5î?ê¨üãëÍ?°¬{6(ÇO?½Ï°ŸùÏ?ªÛNÜM?±K~Ä7q?"LQ÷ ^P?èŠOZR©?£­W-Çw?Å1÷¸¢"?žO]"bµ?"¡Q—ùæž?¨TG'‡|?ê¶Ë±CÚJ?Á®Ž¦Ôô?§(SÂ?¾vòòà?Š.—q\?b˜j^?é–ÁŽ'cü?Âà%FWõ'?È´øù?ÂÄyÝøª\?¦/"–?žôìóÖ{?ëÚj€b¢?®Æ]KNvÊ?¼!ãã?«ÓLܑ5Ô?–òßIëË/?$+'Pôá?郚ÉðN‡?§³W"?Ç8ïL~?¥´ÃӕCPSR4FGL J1736.4-4052¿ï«îÔ<5nÀÔÖ¡aä÷À:PfiÁdºÀ;¿ÎçY@@XÍq7zÁ@²£Üºî?ÈPG@0q¸?·ÀÙú]?ò4Íg&Ç?þ"š™ÉÀ¿à,ƒì‰*·¿âò2ý®A¿íå*ýÌ=?Ó©£Ò؈¿åàÝPþu¿æ!μ'gOTHERunk1RXS J173638.5-405203?Ü'|<g?È&B½rog?n°"òÂÖ?fLi<êú?áÍË.*ún?ÈBRRH?è¸mÏ]Ã!?¾1Ónžæ'?t›Q'¥?†¡ö]Œ?Ìyp¾Gè'?½èywKw3?æ*ÕéÖóÂ?°ÎÑÅ~%ª?–ÂϹ_^j?Œœ"¥
?Ò>'0N/?°6s]'®?ìpKÓ	Ÿ?¡M¹$ݸ?u1M‹š?o3êV`4ú?º‡ÚŒJs
?¡33ú|Š?Ö
Ìd&?Åz‡?{)pBŠ?t;º£¤êA?äÃ	 Ebé?Å©¸~>Ò×?àLÃ}Ù?Ç/ÛFÚ|Z?€G?UT?•úãxšLp?ßU-ðdgÅ?ÇУ"e?Þ ×w0õ'?µL<0ÂFŠ?¡ò{`±a?"<¢ÞìÓá?ß å9~?µý!á2?曢Œ¡'q?¸xZu:–?›j:Ä<©€?•I8Vˆb?Ñ:•ce?¸Ó$'½ËWMIXED4FGL J1737.5-0313¿éitäÖ@-§C"º"À:{i³"ÜÀ<7dè·äÞ@ÆUhgG@üó:õŸT?ˬñ»ÅI?âʹaµý}@žŸj"ò'@
Þ4(Q¿æ²®¨õW0?ïȳBb%9¿Ï_Qߛ±w¿éQß@lך¿ïÿY¢Ò1¿ê8PV×OTHERglcNGC 6402?ã_nê2R?ÂTï6•N—?Ò¸®û´‰?Á¥:'ªO0?¼êH™ÝóL?¶pI×S?Ý䓉Etº?ÆØÎ̝?یzüdXß?ŁÄGA?º;ÅéXɛ?­à¹ªæ[?áüæÖõV?³o¬GyÅ?ÓGëÞØ4?±ëJþÎI?Á°¦óÁ¦?¥ÞÅYÒ3ˆ?âÚ¡ˆó¦x?¡mA²Ùö?ϯl^øÞÏ?¡]Ÿr—9?Äæ
}8‡R?—ÛñÛ`J?ÑJ…¿òôª?ÀÞ}éÿ|?ߝÁ ¾‰?ÆOw3àF?Î0Üÿþ[?Ãûb8¦±ý?Ñz¤\§\?Çm ä³ë¢?ãj¨P§É?ɋTÿ®ø?À™¥n¨Ä?´VEe©—?Óékæ¥]j?´ÒGD&v?àLH")©?¹D(¨œ•?È÷>Ý?­œ
~xý?Ֆ5|!?¨Æj‡-<k?ØsÒv@4_?°û«z 7Ì?ÑöT®O?ªdOy7MIXED4FGL J1739.6-3155?ËžP|^¿Þp"ýþs
À8¤nM]À:X"@pǎŸj"@	:ß.Ï d@_å Ù(ü?×6þ™Îs@´ebZh+?ÿ
¢ÕØd?ܪ(][Œ¿åAxÀÛý¿ènrÚ/­¿ì,` ÿ"u¿ä}C!½¿ê¿ä§Œ¡c'wOTHERsppSNR G356.3-00.3?ÉȖ´YZÝ?Âݤ»‰?¾LŽÍ[Ï?ÈiH	aó?åÄHŽ†p?˲ j‡ø?¾`5ñdÂÞ?Áø×FK?°}ÁuŽt
?¶Ëô´U.F?ê$AÎ2?Ãáâõ€†?Àÿ¦ÍÎnQ?©Ž÷‡¿@?Å+?°éï(›ö?æ{ՌAŸæ?³ë‰P¢å?¸	Îû;¥?¬Iª'k?'råwSù›?žˆ- ú•?ìkEÚeø¾?¯ÌÈ°ˆs'?×@EaÖ?¼t¸y-¾T?½Ç^xÜ4Ê?Ãt¿eS'?ç…n`Ó ñ?Ƕ¼ÄZÒ"?³5ýŽœÌ?º¸²—‡?¹!9ì²\?¿ÌmŸsUì?êuG
M?ÁƒnÙkZ†?ºhV¸jân?¤¬Õ>hw?É.Eý}*?¶´ˆí«¾?ægcàéÔ?¹H"7Õ»P?±B¤5?¶™°Šùx?˜±2+l?¶l8rVA}?í‹AèÜ?¾@ȞPOTHER4FGL J1740.3-3058c?ì}¿¹=ù¶¿ºÒ¥ÿ®vuÀ7ès¥ê
À9¥€!ùO@š.êÏ@E×_ÍÅñ?Ǿ%ÀÕ?ДΣç{O@çžóu®?ó»›~ñ"?ì.¿eÛüë¿ÓƼýÌÉó¿æT%B|¿èm`öºÜà¿éÆ&Tþ_¿áº­EH­OTHERsnr3FGL J1741.1-3053MSH 17-390?"2ð¥ì?"ó0œ|ŽK?©äг8"?¸+Ú¾ƒÝ?íí*"{?¹á-=6'–?¨-
ÌúÎ?¨p"3—6\?ɕ"[ʁ?·ÿSneY
?èæX0
?·îñCÙÜ?³šõop_À?£ŸÀùO¤½?ÁÚ7]S1?«1¸ŽEÑ?é{ža?¯û'‰Høô?{î1'œj?a×#}s?ÀÁ"`2«à?žfv–/7î?뙍Z•ç?ŸyYÎ=ë?v
;~Äs½?w<ß?¥×Ùþár?¸A3µ"ÜÛ?îvmèïJÚ?¸³'ë´×S?'2 ·Ñ*9?•‰ŒoàC¿?Ï7ÝㆳÊ?Àðš
Çs
?ç¨wRL?À´Ré˜Ð?¬ß½­Y›Ñ?š*£ñ?ÃMuÒr±¬?®Þù5¤‹?é^¦°r<ø?°Uˆ<òF?Zˆó˜Yy?IAÊÜ)ºU?ÃO£g‰ã)?¤…J–™b?ëÓªÈÊ?¤œI‹ßþ OTHER4FGL J1741.1-5341?Üü«\d¯ØÀ(¨"1¡À:1ôú€5À;¼K±¯:@n¢ÔUØ$@t£%3–0?ʏ`Fþ?Ä(©båR?ø'›k*ñE@MGva0G¿ÑßrV^±f¿éQK·Žw'¿ä€–ÉÁ0¿ç||Šiü¿í^æ¤h¿ïþÞ&'dOTHERglcNGC 6397?í´±òù(Ã?ªàûêÝß
?t#1k.Ž?Žº®5^»à?¬×Ø£6?§8Ã¥b£Ú?ï8{¡Xw2?"?ïÎ?u½š¯‹à?u½"^@!?"% ÏB?™ã¶{Û?ìswÎe·?¢£ºÄ\qã?—Ìš=|Žü?Ž!"6­?¶qûR? íÉÎhú?ëËl†™•?'ˆÑ]Š?"Rܬúۏ?pÚ@@ xÃ?¼Ò•pŒ|r?öi/B?ì¯CqfA?²Ø<Y±þé?œ³wõLK?–Q~
¢?¸ÄE›"å?°dóà:?íÿ	âú-%?¨Ù=?ñM?Ê[E…w!?"Éþzêð?¨œÊûŒ3ó?¤Ká"àR?é"
H	{v?©ÐÁx*À?§AOV"u?–$rÄüEw?ÃãwõL?§šQ|?åü‹Á68?¥H—·DÕ?¥%4É´Š#?‹`ñŒ"¯q?ÑbAä&Ì?¤I†Úð¾ÿAGN4FGL J1741.4-3046c?ïrÎ0±+¿Éú³åË zÀ9MÛ:MÙ¨À:ØZ@ä@[¸b‡Š@Q¬šþ?Ò±–¡]³?èzÎg×®@à‰ï•O?ÿ³'ú;ñ?͇…oëö¿àZ[–(Ì?×4AðeX¿å"†bZ=8¿ê'Ì®š¿ïÿôým~‰OTHERunk3FGL J1741.1-3053NVSS J174122-3047120?Žwøô™?™gO‹j?ÍÜÃqÖ?Ã7ù˜ª'Ô?èB&Yl>(?ÃÓ Tãuõ?°s'…žÅ?¯MBg©i?É %Ø_Z·?½Í¨n7"ë?穄Y|¯9?¾l¢Er?ÅÇÖBí:?¬uD#ì$s?Ð(Iñ"u?°žÈàº?âyå¨L %?²Î¤y'´?©]§Îå?Š ìØ؈?ǃ%±6æ"?«PAß9/?è‰\!éß­?®['*(?s¦x¡½°?ˆ!0icÍ®?ʪ™Êð)?ÁþDiÅ?èѼŠ¬¹(?Â|¥ÉcòÕ?"ÚînJDú?–Ûå-;®t?ɞ•àZ%ï?ÀÀ†éúÁ8?èñƒieí?ÀE;qMÓ¦?¶&¤Ÿ" ? È]²zË?ÒŸÀq—?¶QH?E¿?ä-[‹þÅ?¶UZØ@¯??±ãð?v'€¸I•?Ç?«hÆ_m?µQŒö­?é¯+'å»ö?µ»."ñÌOTHER4FGL J1744.5-2612¿âñH"K@?ú«‰†&À9
	A}À:Óeµf~º@©Wn¦Ñ»@'û'½?Á}Žá"¿Ã?¸?YV†J?ù•œdO4ñ@2¯Õ›'Ž¿¶̶Q‹8?ïãšn«¯¿æ÷?ö:.¿åµŽÚù¶¿äÁN·8¿ÜžWn{ޞOTHERunk1RXS J174419.9-261230?×åÉ?À³ˆX(¶?‰*Œ]«]»?€ïªD]#?äÈ[àÕ?ÀøåPô†?âoöxue:?ÇMP]îü*?žê.«Ò?œ¿Ëތ?Ù1qÌûŠ?Æï£'Í?áÀÅW†?·=×=HrÑ?ª"-û®1?›F…:^å?َ¶IŽ?¶ayDI?á9Íi"©?§0¶­
?¡tàSqª?}xɚß.?Û]ÉÔõ».?¦tŠæë«?ÌÚÙRÊ°Æ?¹ÕÜ7pQ?"×ÿÈÝ?Œkb©Oœ?è0ÒëANv?º®H/øç?Ø4B¸ób?ÇÇGŸ_?¬¡JÅd?´éa¢W9j?â2T:Éù?ÆäO$
?Ô¨GjUfí?³š¤<§ÿ?²&L	·Ç?¢"F"Â}?ãgɹÐy?³A‡Ur™?҂—,Š€*?«@¯ŒcêÐ?«¤Éþþ?¿
•¥Ü-?ågЖ'l?¬Í¥MIXED4FGL J1745.6-2859¿Îqˆ\Ê7¿£ï›ƒÔ‹]À5–åápÈÀÀ8ïlÒÐ@ "_§ÛPÉ@…+%G¸%?˜…ö¤Œ'É?ÅÄ¿b+]@/
'Ä"Bh?î•‹Â|£¿ÀÎÊ}è
E¿Ú@ "®¿à&cvÇÝz¿åßEuU¿é<ëج¿äç›O|?OTHERspp3FGL J1745.6-2859cGalactic Centre?¥ú¤[Ëu?¿c7 Â\?Û·±ñîß
?ѤãáÞ¤2?àÄ|Á>º?Ñ´…‹ß-?q)è
­Õ?DU©V?éÉZ™uÿ®?½¼¦›Ø±?ÈQF[P€?½¬ˆ°Nx?¯-Ø{·?¡(ud[?Ö:£7}?·ÌlÿÇ£?âñ©\ý~h?·çJ|èîG>åíi_Î/>ÝlrgT?åi9™m$?µwõ@D¤Ü?Õ-`ŸÁÀ™?µwãm¹q?§".`.¡¦?È›Ã?Þñ§tpÎ?Ðãf«Ÿo`?Þò¿¥œÝ?Ðæve¦¼²?mè(9ÜLù?ˆÑóc?êÔ)«ã?ÀöÄØa«l?Ä7»DÜuY?À¯ÅóÎ?§¹Od¾±Ü?œåHÕÂûÏ?Ùͨ>øä?¾æ+Ô«N´?áü5¢Và?½±®xÎÈÐ>ºFÒÑÊI>·R½]uO?æåch/>?¸K
î2Ö ?Ò5¾´—]?¸K	6â¬MIXED4FGL J1745.7-2506¿ï¤»=O¹?ÿn$…ñF)À:,]VlÀ;À9'ÈÅ@'9òj@yÁ­?ÔöíM"‡?'xë¤@ä5À¬-?úϽ<¶ê¿ïþ~üà;?ïý±Ü†~4¿ÆÐîÚ雿ê¸1Ûã@¿ëð`"=µ¿ðOTHERunk1RXS J174535.1-250440?´µçÆæÍ?³ZՀɖ?Ո êu?Ç äš&ê?â¥2'͝W?ȟë;ç{"?¥Ë‰íßSþ?°Dôéoœ?â0Àãñ"?Ê0@ÏþÛh?Øåo@)»»?ȆƒšÝD?М¶ª ¥g?®pïYÔ,Ÿ?ӗ¸‹Ä'?°[›Eæö?ÛÌ6S–?±t­%¥q?±¾úE£?"˜G†'°æ?æœ]ÀiUô?®²œä–†Ù?̯?ª!/nS?©úVj¨'?¦šç_eºF?×Úv"ñòv?ɍ‹ˆ?âs$¹.¬?É3xÏñ"?›'»#ŝ?©m8!5ƒ?än@ò°Ù?͒zun?Ö?÷ËÂÐc?˶&U‡Ïu?Åòó}Ë$?§a¬ 

Á?ØB‹£ÀA­?¶³ÞVßv"?ÜÃú·ØÁ?µ›Üµþ5?"ùd馲?¥LX²Äo?çë>‰Êææ?³ã	L2r>?ÍÓå
íU?³>¾°)MIXED4FGL J1746.2-3342c¿ál×m©jŒÀºAå}»À9¬.þñGÀ;ÑÙ|¸@ôÔ$"ï"@Çz³$…?Ð졾×Ñ?¬Mîd;Í?ç+8ÞøÅ@JÏz?ï~E뜛­?˜¢"ŠwE¿ê)æž/*¿äDïž3h¿Ý
Š2‰~¿ßÃ	Õk׿OTHERsppSNR G355.9-02.5!?×hŠ´_©Å?ÆPmï$?mí¡ Q$O?eçd1f­?ä-Íw€b?Æ l;èc?ãf°rÆh|?Åo¥KËÒÉ?€€óªÁ?"ú!f#—×?Ø®—}4´?Äúð	Ž?âU]E_}?³rä"û¶U? "pÐõé?'ñCÛ|?ÙP÷Èè«i?³|ò?æ.àøÈÃ?¤eîò;œ8?~/'|W œ?a
uS%+]?Ó)¾±?¤I^¸¤?ˬ	ïÔ
?¾ÐÖO`!?u}Ežd?o@o»Xj?èê҉z<²?¿
#1»í_?Õõ+¢èo7?Ãr–̃ã?€£1ŸìŽC?ŽÃ¤d`Ã2?äÂÝgϝ?Ã.šß·,Ÿ?ÒÿE.w%•?²%\¿b+?¦˜ó™Å?"•™ˆ;s*?å£Ù…å)?²h6ßGö$?Ù¾Sce';?­ÕèéÞ·?ˆ€u<_ZB?vAcµw•?â¾Ôyixj?¬ÖM
«¸vMIXED4FGL J1746.4-2852?ŠùÌ=¿½¯+ÀçÖÀ7b·«cÀ9¨ä:§›»@ €$±0d@­ÿYçÒã?¹²Dxªâ?æGa=‡Ÿò@'¡"¬S±?ÿò©ëJ¿ïÿÖ_Æ	?ïÿu–…#¿É"£{Ѹ¿á͚ݼ^@¿ì–à­F¿ëÿfèle"OTHERpwn3FGL J1746.3-2851cPWN G0.13-0.11?–¸4žÊd?»Äòa0?ïpl¾^?¼#æà/'?}f÷@ußS?—¡SVŠ?ybu)p'a?È"O'ˆð?éÇJP?º@çôƒ?ȽÐè°¿?¹õßÍ|í^?¥é%ð2ý?žíגP»?æН"h?µ'_X·‰?ÏC@m>­÷?´ñΔ0?!y*-© ?ýÑ&O<?éÝ>Ӌ"?°q–E¿6h?Ȇ¦f aÏ?°pÞ1Î?–î·Ä?À‹úÁõ?îÐ"ý'î?Á(¡"Ä"?Žoä pPà?¤Æ—> Y?q~ºkrõ?‹Ì¡Ê8ʁ?ël‡
%?¾4å ;ðØ?ÁÃèŽÝB?½ùdÛKë'?œ'¤Õaò?—°ôB÷:M?çyKeý?·,(zc§?Έ"%ÐãÍ?¶8Ò¢`Œ>ì>(j´¢T>åˆÅS…0´?ìyô~'<?«VÞÉy†)?¼/~¸^Å?«Voñ|PSR4FGL J1748.0-2446¿èg£Ho?û&òIÀ7C¼¾aÐÀ:ˆ?›÷Aë@H@
²@ú¦Kaþ?¢ô2ÂJò?Ö'½3Q¼@0¹:>À/0?ú¢3'ÒÑ?î°Ý$•¿Ñp*
ag¿Ýù˜kñk¿ä¸–IƒÑ¿í_›¦º¿ëVxHOTHERglc3FGL J1748.0-2447Terzan 5?G&2Õ®:?Hz~T¸?í¹ç[)­Š?µ\üéFÁ?²Ú×r/?µ<ófV°˜?}äýríju?–ÓÍÎÓ­Õ?êÎO)£?¹†p;w0€?Ãכp<È?¹<±Ê',?ƒPÇ×9I7?‡›ÕêõÛ#?í¼aØb,E?¢Õƒ°Bü?¯e°‡<ŒÞ?¡¢ì ?,"Fò£c+?EÝTÓ?ëå$5O©G?¡·ôý²6¸?ÀdJ .ì?¡³Çs?¿h?Vd¢æý)&?Pà7"'U?íH2fã™?³QLNORÕ?µdÚ;0"Ø?³/ØVÍÿî?néè,tá'?x2%"@ ?ëÅ£ãÊ?½KÃÞø°?ÀmÈÒ¹˜4?¼é·©¤ÿ~?sâVK7:?rÇ$–ëÌ?îB _AÀ%? ô¯Nh—?©Y¯C°÷?›Æ&D¬:-?WÃ2=Ù?2»×t¬?ëžYFdµ¯?¦f݂@?Á…%vå˜(?¦f(B³;©PSR4FGL J1748.9-2021?½jy4@Ç@X䓒ïÀ8íÿS1Ö<À:ä	EùßU@§ïŠçÐ@¤ê/´?¸(^ÿûßp?Ò—=í§@=Ÿ¿MˆI@Åì•j
?΀%)ZAj¿ªnSà&ò¿àê:†ä‹¿çt7ª'8¢¿ê_gJ¹¿ê¼2€…Ì]OTHERglc3FGL J1748.9-2021NGC 6440?²˜XcqÓþ?ªß
'ïôH?áYÀ³[Y?Æ?ï¬ÿ/©?اºdüj0?Å{O	[&?ÃÌ÷½Äϱ?¼"ë@¼o?ْðîE1?ÅEŠÎ¥•?܆"3	Rö?Ãóœ9±ýi?Íß­Pl?¯Ö(h®?ÕtÚ{Ð?²©ütׯ?ۛOÄ +?²g"8ܕ?Â=Õ©üN?"Í¥dÓê"?˴ƤGP)?•ArÆß?äƒXìoU?œ~†*Âo}?¦¯0öì%Æ?£$(– ?â+4¨Ä°?ÃüƒÖ†+u?ØÓ±À#h‡?ÃCÒWY?ªŠ zG?¬‰´ÈiÓ¾?ޏ¡?£?Ê¿ŽQ͟?ޙ«Í£·U?ÉjH™ÿ?½I¨7
ª°?¤¼ÊqäÚò?ڜ¢3àú?¸ixOÙo?ÞóÞ´Z?¶ÍÚb
p"?¥ïû,
"?'dF›+ÕE?Ñ>ólT?¥ç•è m?憗"4Í?§/؇ÅMIXED4FGL J1749.5-2747?ÁôÀ9t'¿Â1²ªŒ°þÀ9yòìòBÀ;gÝkí@Õ±šl(@mZ˜?тl¡"ãø?ïÚø4H‡@~x?'æ?ô‡×¾˜?ï5ø_w´Â¿Ó'óÂÚۃ?åDª¿[Ë¿âÕub'¬¿ì/bCA¿ïþŒ}QdwOTHERsnrSNR G001.4-00.1?ˆ›GpaO?"Ô	P7…:?ÅâÖJ5>Œ?ŽÆX?ê'9qø?¾€¢§µ?Ž'dÈ?•·6§JËð?ß/²•iW?Ëë»Î*x'?ßÜ=?rþó?Ë'ó#£ž*?½ƒí¾4?¤æü'TÖ?ٝÉTaà?´°¥ID$o?ßr/a0`?µa¿IÂÆØ?…³°ä<i¹?l'_¤‡ ?æöëF'?µë_ºô´Ó?ÑdŒ;ã?µtÂq?~?Œ—¡ÀÜ3?´.¥
w8'?Ês"`f6?À$hP]?èðÀ`DŽÓ?Å
–Ú«k?~H`A`Sò?†¶*ÕÞǶ?Üj|Õ,†‹?΄7ƒ`-x?áŽ0ÔÖ}ó?Î(¬?±²Öf‡?›"6OŒ ?Ùg?"E9?»K"ú<,è?á)Ê>ې"?»ä<ÄÆ2?dŽ±,·ê?T¯ç€®™b?çŸ[̞B?¾BÛá~Š?И+ˆy?¾ßæk@MIXED4FGL J1750.3-3702¿¾!ÈoÎw¥Àäõ8À8êõÚPÀ;RՔ«@&¦ßh±@'~D©}<?³éçdӔ<?ÑçäÀ´e£@AkÛm@ÚԏŽÓÃ?ïÿ6A­?ÍÝ%OšÈ¿ã
œ5ULc¿ç4"䤿ë68Öá"Å¿åȊ³LÉOTHERglc3FGL J1750.2-3704NGC 6441?´ÂC毃?«Ö—5¶?ÞfE¼B¿?ÇÈ:ŒûÊ?Üi)JS ?ÅËæë(yé?³,/ݓ?³$£Vˆ?áò=ŒÓb"?ÄÕÇkÓ§v?×P"!Cu?"ÿbÇÝ?ËàÑˆ?¯gÈ_V‡?à]ÃÆz–?´ïð–ÑI?ÑT0ŠG¨F?°|~OU¢?È1]m÷ÝÐ?›ÜXmðÂ?Ú@	‹€?¥ôíBÝ!?ÙÕ?ÿ…˜?¦^L¦¿?Ýƒ§Š‹?'Càµ+?â´åì>¾=?Å|¤Òn¬?ظ[íwÎT?Äç{—Ùƒ?¡MþX¾¨?¥™¡Ì?äÕa	Éò?ÈðP¢&Rr?Õ®•rK)¨?ÈúP#êý?²¸÷×Pf?¢7
äLª¯?å,Xßä?·BZµCžY?ÐùK–p3?´qQ¤Rÿ-?±S…\º"å?‹©ÃˆUy"?ÞebvRþ¼?²s苀bw?ÝE¼1ôï¬?²ŠT"¨PSR4FGL J1750.4-3023?Ú-Ѩøî¿ú'Ã^À9÷q'ÒüÀ;hšQO}í@º†è¼í@Q~B%>~?ÒËUhè æ?寡]³9~@lğá§?þxqƒzô=?¬Ç‰£'Q?á¶úc
¿¿òØ`eÇ¿è¦Æ¨Æ]G¿ë7V]Ú¦ª¿ïïwAU	óOTHERunk1RXS J175019.0-302654?¸©*÷ž‰M?¬q—Gß܂?©³§ ¥F? ¹úàvñÑ?ëO .秢?²3lt¢ˆ8?ÆõÅ©íϧ?¼ð^;8?¾§î3?³ty:Ï?æmÓ2¨°?¿;¡!^†?Ϩ'ˆlåJ?¯t¹²¶?¹i±–} ? ±)&k®ã?äè¥{$8™?±[݂ê™?ÍnY—ÿn=? 
Ç'—*?˦ —~{? ÷6h'ùÈ?áºÁt©ö?©ã§Z§ŠV?§ŸêŽÑ*?˜Ä¹`'î³?´M=[¼P?ª@jc¿ü?ìw¯u4F?°‹ñž«?¯¼‹p'ãh?©PÔo2±¼?¿ÜæNÂʄ?¶q³…—ÈÎ?êšû™?¸e)¯Rž?½éæß®·õ?¢TØq,´?·ì#Ía2¥?¡ag]Ž$?éE>ªy?«ð;ý1Cš?¸ÂV%vh.?– /§5Ú?́xæp·Î?«ØìXÂߚ?åÇW"ø†?°X¡£ÜOTHER4FGL J1750.8-3106?ê¬>	Ù{:ÀÊ÷?gÀ:h²qôÀ;®†Ô@o|—@V[~«×Š?ÓTo—4?ìϵIùHV@©ôafLe@Ù –¦¿æE"~°	H?ï‹ÈUnÇ^¿Xøš$W"¿åÇ-»úír¿îÁÛ!yLr¿Ú–Ý&·#îOTHERunk1RXS J175042.7-310312?¢ég ñHI?››ââh	?¼ãßVð ?´4K->Œ?ë4í¢Û6È?¸Aㄇ)?¸A%_-A?³9«É.?Ԟ	Zã?Ã
È{À{í?â¨Ö…Tµ†?ÁWiÖw4?ÍƇ-±>&?«ÉØ>¯Ž?і]W§Y?°Í·W'€¹?߆_є?²Ž264Ϩ?Í5ÌÁ?¡«g˜Îh?ܬø1» ?«ì"µ´??ÔÆìè9ÿo?©ÂUgŸþ6?›=	¨^ÿ?"ˆėÖ?ÁñxaÕKæ?¸´?þª?꩹ÇXæî?»\aC«•3?¤+-ä^™?¤Õ½Ü?Ք1_ô\^?ÇÒ¶—gvm?ãó4~sÇ?dž©8.V?Á¯yÍíª?£ÉÚ6ê8H?ÕG/ñו ?·VÞÒ~œ?àð‰"Î9Æ?·Qèۂ9"?µùˆmêl¯?–o¬F€©?à¯;6˜?¶]å?Ù#'nk²D?µ]À·êMIXED4FGL J1753.2-2848?â9Ž<_¿õ¶2ŒDFÀ:^ıuXÀ;RU.‹.@'Ê'š¤‡@8Ã`<€º?×íK<¿N	?賁6ÌDè@
*=DŸ@‹¤íµ¥"?ì€BŠ3ö¿ç)BïhÙ¿Ó•j \×F¿ã«LŸjéÙ¿ïÿ»×²¿ÜŽÂÛ²BÞOTHERunk1RXS J175328.7-285014?²™A[\J˜?¨­HÀ;®?½‹ˆ´Äî1?¶ë¦<ŽRs?éûf½›£×?¼/åÿVjx?ÏÖ•¡E?Äxlšª]?µð™5ˆz?±TT‡ØQ?åLg:‡÷l?ÂI6Tн?Ò·²vړ?±Eƒô'þ?ÃZ酕+?§Ž€Ž[h?áÄP
½
?³E…&Ð6T?ÇÃκ–G?I^RL§C?Æt‹á'Ö;?¤¸È­Úù?ärԐÕ??©&ª–~ø? Â{NЪ?˜¢‰Ú?ÂqÚºîu`?ºè^×.ƒ)?ê[m)·-?½>X{þ9h?²}±`??²K§¨ï?¹c˜Ê1?·'ã'ò?êƒÚЛŽf?¼ÑÓ _?ÃZxœsê?¤·n¤u?ÅòÚ'©<?¬K¸ÆG±÷?åølªÅˆW?±@¹õjáÜ?««¾‰bö¸?Žþ²•?ǖф'ӕ?¯Ù¥'%|?è_¶R??°ƒY:쫉OTHER4FGL J1754.4-2649¿îCL®.|¿ãåjR"À8ôç¸5fÀ:R¦'¦`Q@T\>D^T@(obŽj'?ÊÉÓH<ç?À˜|¹)?ü}[
Ѻ?ö­…¼?ïÿ%¿Ø·¿æo—@G¿æQî¿æµV¿ç¦üX«'À¿ä'/ÿÌÿM¿æQµ4)Ó8OTHERunk1RXS J175501.7-264954?")j/ê@‹?'hõqb—?dÎÂaä‡?exC&©¹?ïQåì6'7?'|Êj—¯|?ÀtQ8´?ÀÐ&ÿVþ? ºâB›Ÿ? °8¶b¥?ê×LÇÑ1Ù?Á,ã/\0?ÃW'ë#Ç?ªÖº.·
ù?³"¼çP{?¢Ó%ºüJ&?èɎ߯?¯åìp'³?ª›¤òÏQ?[aîÄ?à"ñ‰4?§•¬äGè?ígA‰†µ?'hLì?‹Z¿ßÁ€š?"`'q?^óݸ¢\?_¯_Ót¹?ïƒwø¥?†Îé‰P^-?ªØSHêd?­VöŸÃ¥?¡óúj;¼?¥Þ±Y\pL?í3;+O9#?²¿\S?»!ÿ;×>?¢Ò0òA?°è|o"? [cd9¢?ê~̲(dV?©ÆçâÇ{?Œ³ZW[ÓÞ?w2X\óW?žƒÕÜÌ?…g:¯zí·?î™çŠà'?Šin¢Í¢OTHER4FGL J1755.4-2552¿êkHJëX¿Ól†á­¯À8>¡%À:"Où<—`@ ,&dä@ÙYæ%cg?Ç2>@­o9?¼Êm!¤W?þKZ;µ¸´@Û´¡ö?ïø׊•ñ¿ÚN`ÐTí¿è#¿dTh¿åÞ$ÿ¿éó`µL~¿Þ¤pMOTHERsnrSNR G003.7-00.2?­£
"EÐL?¦¹™èi£l?"¯Õª®`?§Ûպƶ?í€PzõGH?²t¬>'Š?¿¼)ÉI÷?ÀDUU®?šô:ÛæH³?èÅH@'ô?ë0Øð[?Àr[´~×?ɌZÁ'œ?°œÎ`?¸àÝ(M@?¦kâ@^?æ€Íªdºa?³ŸŒÃ_u7?ÁgóÀgÊÑ?–€Ï7$?•Bxþ÷õÎ?t2!
z?êûïH3Í?žÇ:îfÆ ?¢A³r'K?œ2÷èɁ?ƒH
ü?…uðµZá?îŽÍܨs7? ú©Wfi"?±7Q?±IT¶æ‡?›y+ÑDJ?£Î'–<ƒC?í#µßô?´`Öxë?ǛO?r ?°Êj€+}?·}Y´?§4z¤£©?ç6h|¸B?³,Ç£¸?¥ZËÍzE?…´ ¶7m?˜ß¡¨Á0¶?'mO.&‡?íãV5¹Ú?'äá=2•OTHER4FGL J1756.1-2516¿×FHj8>F¿À;÷ÒßáÀ8U®mf4èÀ:!vjNR@ûHŠˆY«@À	‹û?Ã}˜F³B¸?Û[Ÿ"š‰¯@²¹šû@è*~XËs?ïÿy'3J°¿Õ:–9üÑ¿áôÌÆпëêry\ã¿êDå!ØAö¿ïÿ) 4ÓÇOTHERunkNVSS J175606-251909?•#°ÛßÍ?"ûñ·ï™K?Ç×ΨÅ®?ÆBÀö;h?é`ôHUž?ƓÎøåÉ7?« ™"êw?¨ÏµÅ«7ª?Êñ$+>®?·d–Ck1?çÈ:$?¸	¶S?³iA¯Ý.Ã?¢­j?ÍŸ
ˆ?²qh›FƒL?æ2ð°Ó?³þi‹‹™9?ŽÚƒ$ÕOè?np¸Ó/bO?Énß35j?Ÿ]&Êå¯?é(Þ,èã¦? #¦Ò"?ƒýxÄhvu?Ãsx˜Ñ?Ëÿb\|¿?ÅE®9R Ñ?èëŠD¼óf?Åxº;$w?'-Ú=T‡?–ù¥îŸ;?ÊrÀ©uQ2?¾ÒßÝ"?èÑáe(?¾<Bô.'?¨s,ú¨?™B4™>õ?Ñ3«FGë…?·÷ÜhµÆØ?åÞ÷œ¯"Ã?¸§–éXL1?kßpA÷;I?T ìZÄå'?Ïj*²yO?¬zX¨æþ!?è	•ãV§?¬›êИßOTHER4FGL J1757.7-2337?îJè$?×ó*š}£À8‹
É^çÀ:¡žJÙB@ å[ºà
@ä=F²kø?ÊQù\wÐ?Å*©÷µ®£@Yí{ì
?òe@çPܑ?Ú[©ôÓ?Û&º>ƒ¿è|X@2õ÷¿á×L¸?w¿í¿5դ⣿ÀS±OTHERsppSNR G006.1+00.5?¡"û–j?¡Ž0àÁ£?­q=xÊ?±Ð¥c@0?í 2©º=?µ½¢‡y½?¡\ÕUøÔ?®<˜aà?ÃìA>03Ç?º©"c,J6?éï"[/â­?¼xfÐæÚ7?·â‡R%Y?£ÊW2´?Ç&m§ù.?¯°ñ°$à?ç>ô"K‡ú?²™œÞBw?'½.7#l?tFâ!#º?Áº^Kyó?¡òEî{è?êû£VåH?¢äŒËÄ©? 9L²9›?–~æDU
?±O`•l?°þ(JÝ?ìÒ"cÆé?³qâíã€?Q¼xPO¢?–—s…¥õ1?ÉÊ\Ö«Ùô?ŌYCXð?é!ØJŒõ?Å_±¥mÒ?²ÛùO1¢'?ÈMÍmz?Æ:ŽËy){?±=M
Î.?èÝ# q?²RªÌý?u*ôø?aöJ
V,?ÉЙ
'¡?­'#¨ž?êóQ…Ñ<?­ñÃb|OTHER4FGL J1758.6-2404?ê<°E¾·¿£.y5}À89Vº øžÀ9þœCc@ äÄ£³xé@×î['ÍÍ?Àa×5†t¤?³sæÐ_~?þ>ɄBð@@ãJ膑ª¿éJ]ò#ž?î"Ó–ëip¿ê¦]¨R¿ÜÑÓñM5¿áçj¨† ¿í×ïunA&OTHERunk3FGL J1758.8-24021RXS J175835.5-240203?«A§ÜJ?£ƒ"ø2˜?ƒÄì¶{—p?Š3ï'_ó·?íÿx<–x?¥úʏsÈ?Éqå¿?ÇÝË£Õ÷?œ®b¼SQ?¤
%:?èÂñLO?Ç|{µœÉ>?ÃÙÆÒ¯1?©rÞ&¸çÃ?ÁW©pbz?®ìcC…â?æþs£ï;•?³Sƒæ5í?ÉYö7÷‹?¦¡#י±!?Ÿ«¢€	?'±Ÿâ¶R?èÁ¼%¾35?§ÕéÇ}"E?¬ÇuJ?¤âWwš?ŠÊ:­BF`?‹Æe‹¦g?íԚ¿\æ?¨o
G(Hú?Ä,ö1ŽÝ?Ä?y¿«ô]?«~HRo³?¹@›±Kçà?é<à2žŸ?Æ˱¯:Ï?ÄG΍c¢´?­¥‡â­¡É?¿þ@*pª?¯]ƒE­ ?æîDWY~?´ÕŽ†»Òq?µ†ÅŽÏm?ìn 'Ç?¦À,'f?'ÄnHKâñ?ëîËK‡+È?£HëÊuOTHER4FGL J1759.1-2347c?î\ŸþÀ?OÃ%ãÀ8£hQ"1ƒÀ9Ò`8Nûç@ ½}mi
@"ã^߉h?Ô~/%1'Ê?Éèâ'q	@	Ãa@O?þþ¡ì#6¿îˆ¾ªö
?×ÒíbÄp]?ëéšbí5¿æ"¸žÂx`¿è³†_€>¿è-@ªêúµOTHERunk3FGL J1758.8-23461RXS J175851.9-2345110?˜ÆwÚ=^ì?¡ή|ë?²8iëx€è?Ço°qÍLÏ?ìò¿zL¼?ÇQ3]Yo?ª¼mM3>?²@‹¸ã?³€‹‹cöÊ?³i"[4}7?ëä'¹Ï¼c?º|­À?³ýßpÛ?¡²+®l?ɖ@>¤>?±Iç|©Þ[?çËôÆÍ?³oäÉ=­'?š}¾[jÀÛ?‡¶†xûJ?—]:él?‹àhÌLh?îq(5ˋQ?"tAbö?'B"J¨£?ÌAÙá¯?§Üÿ[%§?´æi¦UÍd?îqû´°?¶€
Ï­Jþ?¡¿""6ÎÕ?§Á+	Me?»7íh^õ??ÀD´"5›\?ë}
	÷®*?Àþ¦1Ù?®Ç'@Øäè?˜¥oÜHû?ÌïF^ߏ?¶g)œëåj?æ×µDV,n?¶­Ý?…!­ðUÍn?y£%ëÁ??—h4û=D?—…åA>·ì?îð7 €=¨?˜ÿqB§3OTHER4FGL J1759.5-2312?ïD¡x=Ý?ˀæYæ¦=À8©¢ò(§À9ÐaŒâÑò@/°NÜ@ÒÇû¬´)?Ò`ÍX
?Ïϧ¹õ@	àÛ'£H?ýI"='Ûà?êo€Á[€¿èìßý+9j¿àõ\"•¬$¿ç÷ÆÀÄ*è¿æOæ'æ¿ïþ'!€-bOTHERunkNVSS J175948-230944?¸¿%®êi?·€6¡î?—zë+þ"À?""?iJ½?ì,Dwð
?¹ÍÒQ@?µQ'¨"Ñ?¹.©ñâx3?ª.`O€¯?ª!P#,J¤?ë²ö+¸7?¼šÇAªÜ?Â3'-?«h^†o±™?¾~÷¬ÊN?¤—Í•äG,?ç°,AËÒ?¯Üj®™ò?"ƒ®µiH?|x©iXÅ?Šö»(Ô?ƒ¿F{Ϭ?îoŠÙڞ¿?ŒþŸh÷¡?°IŽïÓG?¬æÃN5ýo?•"8cS?•Òa€0c‹?íJ5˜4·?°Øaž‰ -?£c$™e·Ø?§ºÐh;<g?±°$…df.?±ó*NÞ	‹?ì"É&Ïì?µSb†:ŸÂ?ºÌø>b?¤V‰Ã~>?¼LF'?¥X/î}'?é"õ~OnÜ?­•²$óÿ?u7ÉN r?d¶ÅÝu?œþHn#Œ?‡!Gò^·?îõiö,±S?ˆ¦¥µu‡OTHER4FGL J1759.7-2141?F¤Ð
f0?á)À8Ïa€M˜9À:ªh_dêe@Àîó[Í@¯…^y2?¼Ž½Gž¥?Ñ!šÄçÑ
@ÛHƒ&Ž@9Çóʲ?ïþ–Ž0Z¿çôÛߏG0¿Ùzßð&¿å2	g‡Î–¿êC@؍J¿íû,áàZHOTHERunk3FGL J1759.6-2141NVSS J175946-214231?À3«"—!?¶Áxlv–w?Å4Mw=?¹Ÿ¿9{?æ¦FÙê?ÀÚÒÀ	?À׿¾‹/b?¾|¡âÏ~¿?µ2'æïZ8?©±õªlý?é#½³Ä?ÁZ6ö>é¨?ÕC…]º?´µŸ«ù»?ÇîÍ)áGP?¬<¿(=n?ÞîUçß]?³ßRäD?Ä©±ž?šbA'p!?¶°žÍ=¿?Ž-± Ýè?çÿ·_Ÿš1?Ÿõ˜ÝÜ×?°¢¬ñBÖ?¤à§G"N?ɟòN;¢C?¼'¤Ê$Pí?ç•oÒï?¿j퉰ÃW?©&]ð?ª_#áb"O?²ò{Ç.yÑ?±Ÿ·»¥?ìNöv®?¶à'x(~Ñ?ÇB‰Ib?«Ä"Íw¼?Ì?ø¢'e9?°±ÿˆ<¿?ã€&½Y?³<Ôyhž?©ƒνJ ?‹ÞÉ/¦5?½-pÚ`?¥m!}?êĈôÁïŠ?¡Mú"µ%€OTHER4FGL J1800.7-2355?îõƒb—ò¿×É] í`kÀ8<Rô™špÀ9Øïÿ×¼@!º˜ó¬_š@(@Že‰?Ä6¨2¹°?²ðãB1h?üJë!L?úúŸ³ºC?îT)'°I	¿ã.ôàM/?ë^ÊÆbO€¿çSÿ[•R¿ÞI½ƒƒ­Ÿ¿é['£HoOTHERunk1FGL J1800.5-2359cNVSS J180041-235622?ŒL
>án?ƒ.R0 ó?€¢ÛÐ^qa?®NK_­?ïLDf·D$?®X‰úT}?¯'CΆÂD?¶ÍÎãÿùˆ?¥²jœ'-¦?©Û'Æx?쫵@²'?»	T^H'?±ü‡F"&°? ¥YÃÐ*Ï?¼f3Ä0N°?©ô%§–$?ê3¨žš4t?®þNjcX¼?™q¤‰Áó?‡	ð"õg?ÕÄ?ö¦?…9+:ƒn?î­Ä»J2B?';B¢ƒž?‹j©FSÚ?Â.T!xt?s"=.74š?ˆáÊì¡?ïkLàaß?¯yُ™?¡ù$"'?¦ˏß&Y?§Bs'ÿW?±Â®|.îŽ?ílF†|²?´Šdý˜#?¬÷Ç&Ž—Ú?™p!²¤?¼ö/û"ÿ?¯ŒÈØyèÊ?ꑽŽ…-@?±ÍS%.?ƒ4Üò±þ2?wc¡µ#è,?'S›õûT?'"w¸Ä
S?ï ´h¥?" ¯ï—+OTHER4FGL J1801.3-2326e?ïjøŽ¿Ð:ÛGÀ6,l™†NcÀ8³Ïqºû@ »\æzH@B¥–ýÞ?¬¸oâTã ?ÀÁà [R@!,ÁÊ:KU@ºyŽq¿Ò1܆~3ã?ïsR4¿å•"õÎN¿ãÁè"Ïf¿é9Ò9¿âAî¢_ßOTHERSNR3FGL J1801.3-2326eW 28?Ž|§;/æT?ŽÊ:^;BÎ?³[R2?¸1œ÷fž?í$¡øÅÑ?¹î	±¥A?Ž
õ©QP?™¶¹KKéõ?ã£hò ³?ÇS	ÁŽ™û?×ÈÖnÈEæ?Ç#È/äÃ?²E©(Hm?£'6ƒ1¾¸?ăöÂóÛ?®{*løó?è–`ZuL?²^jì`z?Pà ÀI?<îˆ Ë@?À¬¬]ò?¤]¾±?ëÌsX'=Z?¤.:"?\?†MJu>ý^?©[WŽb&?²Åu°$XL?¸—JNb?íN O´Q?¸Ù7œ×ð?€:)0Jׇ?ŠɅ©ÿl?äK{~{†?Î×NÛÛ2–?×O—¿œ/?ÎZ	8ä?«Ök8ᇕ?ŸPVY¨é?ÅÖ$ "?¯fk4z‡»?éãÃ<÷?±öÒª%e½?4ji%–'?++]gP	?Å!"ìÛ­]?­íÂð6"?êµwK»ë?­ø8Ã7o$MIXED4FGL J1804.7-2144e¿à‹¹Ôøj_¿¸G7÷é=À7d/TbÀ9J®¯«SÖ@#*0oç@UhƓ?«R€o?î?'IR{Å?²?ïÝDêÜ0@Ë<quc.?ï÷Տ-Ú¿ÞY•‹–¢¿ç…=jĚ¿Ø9›aðµà¿áCœRæW¿Ðø3£¡ÂOTHERspp3FGL J1805.6-2136eHESS J1804-216?cD¨2?`[ó'|£x?@Ü᧋?B½žÃvÐ?ïèê8v?b¬ê7£{·?¡³‰ƒòŸb?­Ð Ênl?¦ƒ~½.Ñ?©6
 Åf?í'ï/ðý?µEÆiÎ?°Jç€Õƒ?¡'´	{?¤m­›mÔü?œJ{u^?ì¯ÈB'@?¦åLµ
Do?o'	~/»?vê—ëÉ0?Š›bKrÇ?w*ó°{²M?ïÕî^—æ?'†S3û"?oÊëÎÖ~?hÑÅÚ?Bh\jœ5?A¥;õÉ\È?ïۛ
ÚU™?kQF/ˆ?š¶ûü2?£sËø¾!¡?£ó"Lá#)?®6a2l[??íïØ*#,?²Eß=Û?®z¾#'«?ŸO–-bë†?žB÷­h[ô?•7±öq[Ä?í&?F‰H¶?¢I:"ÖÖö?rlüOÚ?dŠ½Gƀ"?"13*"û?†³%r/'K?ïAœnw¼?ˆ£<^×YOTHER4FGL J1805.6-2136e¿åλê§SA¿Êó› ­JÀ7cÿ¥g-6À9A¹d:<<@ Ðyšu·'@žš|îh(?·6=>Nð(?¼¾-]íWB@*{[Àðö@åŠÞÁ?ïûþQ)=¿ï÷" fQï?ï¹ý‡»¢¿äˆk%^¿æ.oŸJ2©¿â󵤒 OTHERSNR3FGL J1805.6-2136eW 30?xl3}XŒÞ?8 'õ¨:?\|Ô§5³?lMþWŠ³©?ïÁZƒô?ƒ;ÌNj£º?¤º;—ßû?­èÒ~÷ޝ?´HÎC½?µŠú˜­£?ì+B~TĨ?º@ý®
'Z?³ƒ©$H?£œ6É>«?¶æùÎ?¤Rp‡OF?겫¹VÎC?«Å·š‡?e==@‡?uðÄãœ4?‰V´ê?†Ìƒ++?ïW¥ýÄÖ"?ŽSÙÞèŠ?†F†SÕ?'}Ô^j?hßqêNúü?|5Ö^Åö?ïŽtÒÿ†?"_Oö×E?›<¶Û#?£­{"Dî?±˜`eZ?· ƒokÌ?ìó½Ý«?¸6¢QV½Z?²/-%cM?ŸIøӃ"É?´éZ&É	Í?¤mú~g¸A?ët?ªaƒÂ\?i}Ïn©µ?bѲþ?Ž2þ0ÒBÉ?''ü\"
ô?ïn‰Œä³?"'ßÎͧOTHER4FGL J1805.8-0803¿±*7*"@UÔ¥ß":À9ůJÛÆeÀ;Šꘐ@&¦7aÁ@Åêû‹üù?È}ë=PBŽ?¨}¡%ãr?ätÌ?ß ?ý­:`N?ïû¶Å#‹ ¿éh°B¨q#¿ígB'¿ÒùsÍÅ¿á	²Û‰ÿ¿ïÿ‰kVOTHERunk1RXS J180603.1-080612?Ó¼·ÔÜÕ?É3ÚÚN?"¦D	࢙?€kYÇû?åÏfҒ+?ÉU¬îË<?ä×ßs~¸ÿ?ô1hz4?›p_ÛÕÏ? ¬©i<Ò?ԙ;E<?ÁñMÈéF?âv².:ûÔ?±ÕŒ p?«h˜³ª6×?ž·C )/î?×¥ˆŒùDœ?±
äRd È?âƒgp?²e=³z¤?'øÍHØù?v6<)â^¨?ÙÚR]G_?²Yé|"*µ?ʏӃ[{?Ã<8{­²?ÊဲÌ?‹§ò_Éã:?ép…ãÞ?ÊZ¨SVû?×3ÂPXCI?Ą¹B×@?¥·Ù¶WO?«²6ðîD`?ã
­Jü?Ãc\͸S?ےý';û?²fŒÑà?²ÚQIé?ž1W¸ï?ßèú†T©Œ?³0Œd©'?Ñî1ݕ?³ ÷N†Z?£ùÛpüô?'3Ú®ÿàµ?åÉX03Ç?´å‰aMIXED4FGL J1806.9-2455c?íŸë¤mÀ¸Ðº%*À:o1çÙÀ;|`¾†¸ì@ÜHjÒÝ@"Á=L'©?ÔjßÇÑ:?êê!ƒ"@?úÁҝÇ@³+XžQº?ؔø T‡¿à39žeË¿É) 7mŠ¿éGF{"¿ïá=¼#1¿ïþ¼3!•|OTHERunk3FGL J1806.7-24511RXS J180700.7-245619(?ÍrsœÒ*§?Â+`ã´_?¦VæÕWLý?¤jO6ˆ?ç=ô«Ÿ;Ö?ý"'?Гþy?ŽfþšWã?»_Dcv?±ÓJÝåG?äJšg\?ÂƬÀEˆ~?Üm#æje?³Qïk?Á¨([F€K?§Q)¢Â‹v?Ú¾Çì=Uv?³"YàSäÅ?Ù7©•÷3å?§hVè÷?ǜ'Rš£ý?¡ŽÎÜ
q?Úú
À»z?©÷±Ð7´y?¼ ‹2E?±D¸KG?±›ÓÐá?«"Ú‰k&©?êXÛ9Åã?¸e¯¶ý³?·Ùžm±æ?´B"ELq?¾ŒÎ#‰?¸ÓGë)ï?é3LUb?¿cÒw܅}?Óõo¶Ï½ö?´t'$å{?ÀæœâEÒ?ªK |=T?áËÃ=_?µ1Ažø©?ÃõÖ}ÇùK?£¼?`?Ïo1pæG?±3Z'?ã&¾Toæ?²dîžo‹MIXED4FGL J1807.8-4340¿ê˜EƒdEqÀ&G2œ4~À:4I½¹3"À<àd)u@§ÏBrì@ùœÝñ¸?Ãi¦!gXÕ?Ô'r 0Œ@
NHboa?ú:š³JÕ?ïù?†þŒb¿á8ýw"¿ÛxŒÙ—¶k¿ä½þ}ÉÚT¿î–q[Œî?"E©'oÜ\OTHERglc3FGL J1807.5-4343NGC 6541?ÓçM30üD?ÄᏛ¹@?³"u(²7?§ÞnºçªÆ?ã™ÊÁQ:ý?Æ'¶À4Ó?èqÌ'éÝ?Åç¨ì?±n'ÜÞ_>?±}±ÃSV?ń[_ÞH1?Á)´¼,8?䕇 Ç?±ú8è®k?Á;ÐCWv<?¦dïþ1?Ìnj&J©?¬Ô_Ü¡'?æ7¤QX5?£ñû_¦;?µXó X÷ÿ?¤Ãݦñ?ÌtôéÌaî?£6Úl®»?Èd<uQ:Û?¼á²ùÎ?¸J6¬Ùo?­ÚùŽ4I?æݪ
7ԋ?ÁZ}'•O?à®RµüÉ?ÍÁßaí?Ä3f •T?ÁJê%€Ì?ԉ§Ev#??ËIìVÄ¡Ÿ?ޕ¦UØ¥?³…¨GF?ÈügÀûÖ?«Íú'"‹æ?Ôì÷©p?²š qéÁ?Û/ýõŸåõ?­åæŒ,á?ÂÜ߃L"ó?£ê?wqˆ?Ûa'G¦îÓ?±§Ðï}C%MIXED4FGL J1808.8-1949c¿ÝPxυË?]ÐСõ\À8ˆF"
qÀ9¶¡Ú°»@ –îE1b@àM/^?ö£©Ø«þ ?Ôôqâ'Ò@Ãñ[øN[?ø±÷¤;Þþ?ç:¶#£s?îêÖ£d!¿èÛLAw»¿êKåM¸¿çqµºa>¿àÂç 5)­OTHERglc3FGL J1808.5-19522MS-GC018?ÄőJ¦Óz?Ä%'°ôÔÿ?¬"VL¤?´sfpu©'?éÉäÌ.(?É'daÃ-?£á?֜¾Ä?°"'Ÿ4Á±?»L€a9V?»OµË\?ëabr³H9?½Ã#Õ$é?¼«»ýi?§Âõ"ûƒ?ÊCS:9¸?³â¼>³d´?åí'3(T?µ•† ©¿h?ˆ4^¨î%?y:{Õ??²òÉՄR÷?²ìë\L5?í@ÕJtÃK?²CtÖ§Ó?½âr!@Ӗ?ÃòjF«ò?µ5'f¤¹X?¿†À'f»?éÏ,‰²?ÊquVKï ?˜#NYlgc?£#X%á?ÇVÂ
Y'?È.'ý‡Ät?éi5
£Çñ?Çí"ÃÍä?¶ih {«µ?£•tˆ?φ e8%?º!wÒ}?åQ*Ò¼zð?»¤M°?«ð?pqj7°?s›pçÒ?[?²˜lÅf?Â/÷¸øs^?흊¿r`?Â,ƒ~çOTHER4FGL J1810.3-1925e?ªÿ¸wRM¿¾(w~¢ÙpÀ7±C΋é®À9"y
2ª@‰Ä7@Š|Æ$<?À<"·Ÿ¿?ÒEkD¸Ã@¼«œÑ\@Öªß<;?ïë>bk]¿®w9>ÝW׿ÜèƒažÖo¿èPÄsa÷l¿ã#Îq»¿ïôU§ÒAOTHERspp3FGL J1810.1-1910HESS J1809-193"?ze q8Í2?rä'\­–?ÚFT˜Ì?²`6Ö¾® ?ïK̵áßë?²R0…ä	?¯Ÿ¤UÍK?«ÚbÆûzÖ?ÁY .ëó%?³ßó~¿?鯽®‡ùo?·XýïšÝ?²BŐ
A? ¬–®O*­?Áƒ`856Õ?¨uŽ\ەk?éVç9No?®4ì›Ê ?†îD'7'?w%Á"ZP´?§ÿl%t?'$Q+b?î$VÇ'?•ìšö4?y²5
È?o'd"]²Â?"¯CPÁ÷L?£Ïë«®F?ï0nVÆz?£Tbû#j?˜Â—Þ'Aó?Ÿ[S[ôQß?ÀÁ#Ѓk?·CݽÅO?ë	¢LŠa?·R.E?«OÖ·D?ï?˜ä»½1¬?À¿Á/¤w2?©DmŠuxù?êH¾?¬M¾Ûº©É?niƒ®+§?b-ý;™üó?¬wH¤A0?œáæÓÏ?î!úP¾‰?žš:¶ÎøOTHER4FGL J1811.5-1844?渥\Š3d¿¤lי¯iÀ8EŒîkóÀ9ã?¹SsE@+×IR"@ŽŽ¾tDu?Æ­'@
Üþ?Ý$)à¤&@ž¡aä÷f?ý	ø`Nt?ïû1~þá¿Ùv}_Ò"¢¿æ"ù2e-¿ê¶CŒ¿ïÿýF\I?ïÿ¨âaßnOTHERsppSNR G012.0-00.1?ÊÖ®­§îq?Ȳæ(µÎ%?Ì-MmŸ?ÉÐlý·ÙÔ?â?ÁÄ0?СXø?¼¢Àïñ?¼â4m'L?̯f± /1?À̑Nmª?å?ÎRšö?ÂàY5j4?Ê¡}yä"?³þá
}j?ÇSyïÛÂ?¯–†	®z?ã¤ù%40Î?µØ+ô§;¬?Œ†‡ŽÂ4Ÿ?txúü6?Å4c@än!?¤¨C\tjÎ?ê@Íb V?¥éÑvqú®?Á?Ûç`»›?ÉØ:/7k?Õ7ƒÖJ
K?Îy'	¥?áGËó?Ðæíª'æ!?œÚó¬Ø?¤nõx‰öÜ?ѽœûpE°?LJùèíG?æ:YêEóC?Ç\º"åqM?ñ–ÄŸ?°GÕVÙâ?ÉRù± 7È?±aݱ¿¤?äËUQÒ@æ?µ»¿8ñ€d?e	ï—M÷?Rº›zm?ËAi2Y՛?±Æ6–«X?é›Ã{¦{?±Üðdw;OTHER4FGL J1813.1-1737e?ížñ•·•a?Åæ­ýÀ6…Fü=ÔÀ9OVcÉÔ@f€®¼š@T¾ÆyÌu?©$S…í?Ã@y—Ɔ@µKHÓ®h?öf¼ýÌÉó?ïÿ@OÁß¿Ò2l"¿¿âµƒž¿åéҁ—š;¿çEsÝGnT¿ß:md1'ÚOTHERspp3FGL J1814.1-1734cHESS J1813-178?w
›ú'5?yÕÛʄ³¯?¨>ÿÃdÜ?‰](:‹á?Já`ê?–·¨Rú?—ÏiHé´×?¢˜XËÏõí?â,·ÁLæã?Ã?÷7•©±?Ú)™è… L?Â`0†d?²˜¿;˜:?¤m‡êAj?ÁQèÕìÜ?«R2Ê$c?éjӞ€¼±?°&ä¦f&?qø4Ûݐ?^WóAO†?Äå¥"†4.?­7¼[šÃV?ꢦM‡i?­ê«ìî°k?}¶Iw+1?x™ò£Ó?¬~Âãrá?ƒÒÃâ8ˆù?ï}ár Xæ?‹pà -?€¨º¦
7?F~â6«?âi@Yrž>?Ë1‹ÔÆ'?Ú¨9x$\‰?Ë
¼:G=p?«‡…ZrgQ?Ÿ4ð Ýá?¿*'ñQ?©€"Û‹ùÀ?êU'WÕ÷:?®u.¶cä2?W!{½Ë?I>RsHE.?ÈÄÅí4¡G?´93Ǩ±?éÃ=Ç-H?´W,¦Øð'MIXED4FGL J1813.7-1536¿ã"®~5Ï?ðŽw&¨
À9rp·"@À:¥Mçê_…@ ^)dÓ@Í`ÛâêF?Åꐗ'X]?.77¸º?Ï8ÿ%­B@Òͺ³p?ì/8"9³¿Ý#÷p"¿éÿJ-J»æ¿âåPQQ+¿çB:73rô¿Þb'|,OTHERunk1RXS J181335.6-153600?Ķº¶8¥}?º]ŽÚš?ˆ-°ž`+?ŠÄ¯ê5_Ö?êr œÓÀ?»
06Ý?Óɹ`Î?̝Á‹dß?˜-ö|VdQ?Ÿ!àYÚWs?å°«o–!%?Ì@®ø6Ä?×÷šOeݙ?µ8 L¥Æ?¤ÚF°¾Ã?•¹¨éÔ֘?ⶎxd{ç?µ'àåi™?Ö6Fe6‡ô?­‡h'|]Ù?ˆ_rÆ
?h
 B¯?Ý?䄺æðî?­†Ò?óù?¸ÏŽÙÔ?³oòÚâµ?ˆBª{gu?ƒS&›œ?ì…$n81?´v!ŠuV?Å}—+;~B?Â&*ñ	0ð?':NðnŒ?¢¤Fûì@?êÅÊÇ[k?Ã6+Ç??Éôoõ—Ç?¬FPBùÔâ?¦ÏK Ë?'á,–'}?èó¼ûžq?®lÕm´?ÁE/'?¤¶=ß̓H?<´¥ßY4?xá—4é"|?ë,ž¹¾þ?¤ìOS»™OTHER4FGL J1814.1-1710?äDñàhÇ%?Ç	j!†ã_À8ò(zrÀ9þªhö‹@ ~JL)@¹åi|?Ð23Xòà]?·åΑs?ñftù§ k@½®€0'î?Û$cAmހ?ìÔ_¾+Ÿ@¿æE^XûÅ¿ê)óÿk°}¿Û]"3¿ëBÇû¬´)OTHERsppSNR G013.5+00.2?¡ZaŠßl?—=~2,o?h¯ŸŽ|åA?kԏ(Ç]?îѪGšQ?˜Ds†ç8ª?½þ¨¼ø€?Á‹6ÛÅtO?–Ph×Ÿ?ž^!8ù‹?덪tՌ[?Á¢/
ùV²?Ãf6±© ?¨	Hâb?½t(­"ñ?ªÃ&/ê~d?çwí=õGÚ?±ÞnFó?Á|/Pz–Ê?¥æ菝'·?ƒ›¦€FÞ?pY¸‡‹D*?ëR…'ìÙ?¦§e!QeL?šr%{("?Ž.غԘA?hw"'S/g?oiŒÛúøé?ï÷±Ûbo?¸JA"5\?µ]™Ú¤TG?´¥ÝHÑ? Ãh±*–?³It»ò<§?ìH9}O6?»‰èK®T<?»'W/*©¼?£›¶sQØÑ?»iµT¤á»?ªÆ@<lS!?é žo†'?°O–'œ?ª€)î[«?™À©ùš'Œ?'"Pë-²?væ¾õá?î
²9ðÞò?šëi}!]OTHER4FGL J1816.2-1654c?ÊfW'¦¿ÁS|©É½yÀ8FñTk'À9Ñ×rB<»@Ô_¾+Ÿ@Ä[^Ëgr?ÏJ*,¤N?ê[éhÐú@-?ü¿ÒxˆQô?îê?¤Z¾¿Õ4Îÿ,¿åÀ ·/¬–¿îo/˜sÿ¬¿à± ‹ü"%¿ïþLké]&OTHERunk2FGL J1817.6-1651cPMN J1816-1649,?¦…¦ÀƯ?¬œÐO¡?²+¡n=Ÿ?¹ÌV&H?ìR1f2±?½wôT$?¸§``Ìå?» óët­§?Çîd†+A'?ÀLI'Øø?æïzҌ²ß?¿!t¯Tkè?³á¶ÓÏ?¤Paù6Ÿ?¾FAǏe?«*Ý
rú½?éÁ]?m¡?±¼è¡f-?zºÉ&†z?cp¢ŽÓó?ÇNÞ¦OEÊ?¯ *§¶w?éöÒÄ!qY?¯~éý$G?•'öP:X?"îñãþ.Ô?³Z3¯Þ>4?·
U¤³dW?ìè¡×«£?¸ïG"‰Òa?›Èüˆ©?£¯téýX?͍"X֗?Å=zkÎQª?çÃÁ%Ø4h?Ädò4²±?­
šâá:? â{kÎ]°?ºåó[Ï+?¬ü2?=8¸?êÒgæeœ‰?²‹è{á?TZÛ«Ph?F9à–?Ϗ&Ñ?»äC>¡®ï?èò~x?»çv'­MOTHER4FGL J1818.5-1656¿ž(Y·íœÅ¿ä¨ªxäî,À8×£Z»ÐÀ:^xèI*@ûÙc¯@÷‹7GN?ÆvÚèCuÌ?ٚcƒˆ
P@2 f<u?÷úÿåþÍ¿ïß4Bý«'?ïû>?*ã.¿à¸Gڊ%¿åz·\Ç+¿ìӋ,ïLT¿ïû¨LºÃ¶OTHERglcGLIMPSE C02?iÄê@v?qø Ïf¯µ?†"áÚâ?§ýôoµ?ï‹ì]ip:?'ÐJ–ãB?²U³Ee†?¯¸RÎKU~?Ï>
ÇÚÅ?»¨°«âz?ååÍWiÑÞ?¼‰)	
Å»?¶ÉÁYÅý?£KIajJ™?Åç:»¦?­u®Ð.ù_?çÃ8T˜f?±éêíÆ­Ô?¢âbÌ–?ˆ™æê†üF?艠¨+®?£'Ä°©?é®t'Ä°k?¨)'JšØß?lééX»†?j¨Œ†ú›=?ž2YÇÜ? [jáŸ8?îñƒH|ú?¡^›ð'4?–dm®Re?šWloâ2‡?ÐÐÄ-–ç
?Â…î
†ž?æäz{Ï·Á?ÁùUýôž3?®$Í
›f?—°!±°±?Ä%>–F\?©í'à>¥Ÿ?é}s{ÖC?¬öZïø'p?‰ÔñTû?tE»VÈۜ?ÇI–î`N?±+•ˆ|‹£?éÆJcš?±û»¿â˜6OTHER4FGL J1818.6-1533¿îb;qáÖ¿RnóÞ)YÀ7^²²$«À9^[ÿÛ@"ú%u…h@;¾òïv?µ7ƒNÿl‡?ÒÿßÝ5¦@1í¿‹›ª@‰a´¥ä?ïÿõ4Ê㿽ë *F>¿çìÞ²þE¿éçÑ—Êâ¿ëŽ5Lèæß¿ïÿò~#¿OTHERspp3FGL J1818.7-1528SNR G015.4+00.1?tHþ[Æ?…ÿ°˜Ç^9?¦c ·Ø	?°X{Rlð?îqª‹ÉD?°¹du˜?œ)ˆÇªt?¡@}'*ãÅ?Ùõ`÷‰o?À{f‹‹u?â$@¥?ÀÛ%'<þ?À…ýh?­JÍ!¿?ØèÚÁÏ?·x¢»³?ßé;–
)?¶4™W?k¶¢ŒZˆ?W#Ýa8ä×?Á½Ëb?¤8|NSKâ?ëtÖ}i|	?¤¨I€]?o£(r‹s?'VŸä¬Pw?·ýTaôÝ?¼g‰f›•r?ìà²a³ñ?¼u4¦?…-
:ŒT?ŠLtçwaÐ?Ûë"~—Ø?ÆÏ[ìԘã?ᵁ»›:ó?Æî~÷	"Ý?´½û±ÑC¶?£x»"yA¢?Ú-9†Uç`?¹´û›}…£?àQ£ÆÄ)?¹(Y'0?J	2ªdu?;ÍáÐ÷?Èd¥ž,á?²x[Īr
?éàTWßÔ«?²…n4–(¯OTHER4FGL J1820.3-1009?²ù&oÞè·@zÿèƒÀ8òdtJÀ:®nƇ8n@x±Ü¤Û@^YåN£Ò?Ç=|!äI?ÒTÕd éo@KBôqW?ó	Gðjâ?ïÖ8ñ¹`¿É68¡1=¿äÛ
bY'l¿åépq'#[¿ê#u –
¿ïÿð懈öOTHERunkFK Ser?ÅíÍ$­Öµ?½Š‡¥GÅ?È%|è"?Ã)
 S-?ä{I˜-?Ç~žòÛ—?½Lç=« ?»{Rö`ß?Òl	,hX?ÃK²•ô?ãR-=Ø0?ÂïřÁvq?ÍÅÍK€e?¯©÷j;?ȹÿ™íkB?®1'pËÝ?â`<æ1Å?³̉Rq?¦F&Ÿ?'!¿nc?ÎÞDÈ ²?¡ÓÈ-o"¥?æßzfµ?¢.+Ox³ý?¼.ïõ¤e?²‰½¢p)t?ÉX†‡vµ?À¾)é)ò?æ7ß©•²?´ße€¸L?¥«¶÷Q:?ª¢á€?Óó™)?Èi°á£?䫸[I?Ç–Ï øÅ?Áñ‰'þ«?¥ˆ²–•®(?ÈhÌÌe¸…?¯ö['Î8"?åijl&ç?²»×z›i¸?‡:ã"2úà?m%£kh"?Ñá­C'?ªŽ»£'h?æ²=Ðx±u?ªaÀŒ¾
OTHER4FGL J1820.4-1609c¿é´HãYè:¿å^®óÀ7vÀ#jÀ9ªdÜ"«&@lúnp ý@RnÚ©.b?°Wá&öå?gêfß´»F?³£</±š@Ý<¥wÉ:¿Ý	üƒ×+¿çµv¿åªÒa6PÊ¿è{:3µ¿ë¿Ôj³w"òOTHERbinKleinmann star$? }‹þÈ¿Ä?§Øã–ÉÍÂ?rùöki?'ː
–?îÒ5 7å?ª!0]]+¿?Õ+®Ž(*?Ñê0ñöŽ"?›B—þY¥?¢:ÃÐmÎâ?ä}Nêk:®?ÑÊÍèšw?É	VH"¢?¯YÝX½?»}—|Ö6Ð?¦&Ò«ɛ?æMJºÓý?²×"‡–=Ã?ÉëyÏé|?³Ö{»Žì)?'–±Ïô´?xÈğ?é'"'Üà?´žA"[?˜~´¢Žª?§ZgP†?sŽáe#Zú?|¼'ûLJ?ïñgm?¨t¹f#Ý?ͽ{ù%?ɏ;€Î`e?¡•¸Î
À?³ÁN$·U¨?çwEu^ƒ?ʋuÊ1'ó?ȳû%8Á?®n9OŸ(?»
‡ "èÁ?¦yçŒúÉ?æq°W(äX?±N2d)•é?µU~Õ$?¤Ï@²‡-/?œ€…Nó}ó?Œ,ªkcÊ?ìqK¥Öúß?¨"¿úˆE)OTHER4FGL J1821.1-1422¿à×3}'ju?™ÎWçG¢VÀ7"H¤´ÏÀ9Y{ÕctD@§i&à@M¢ÝåùÄ?¹Â|ò–‹?Æ®nþ:ƒ	@
ë€ìúi¾?óÒÑ=õ®î?»›Ð>ò.¿ä(@zi¿æ'ñ.«äö¿êAyHªi¿ëát#¾K¿á»]¤ YOTHERspp1FGL J1821.1-1425cSNR G016.7+00.1?'këM¥×?')~pÌ°m?š
T§
?­þîÁ•ìN?îœ8k	?¯ èà' ?¥¡X—Ö'?©çØ+z­?Â2 *KO?´èÀ™–?ê"MßÔ2ê?·¥]B|õ?¼Ï)͝›÷?¥yCވ(?ÈfK¦	?²?Ôð‰tÆ?æL‡ÜDž?´Žf&"õ?xÞ³>cB?h€oñé]š?©>ó/âñ§?'Å/'=5?î:T'ÊÏ?"ýê"´e?€Iø;ü]œ?~hýמ?^%gR%?«	u¤»Äc?îÓæô8
?«Ä	3TC?'JõK Y?"z¿ѓô?þ´m°]?ºÛ̯p›t?ê~#¾?ºjf®¾LŠ?ºøÏÍø?£ãq¬z"Ú?Í]/Ä?µ^iœðžá?åy©§â:P?´ì¢[-Nø?\ƒgOèÉ?Qƒe衛o?²+««ÒÈ?¡[±>—c‹?í¬^hsºj?¡¹Øâ|OTHER4FGL J1821.4-1516¿îï
øÍAù¿Ý5%:ÍÀ8Iûçl‹DÀ9¢*9mÇ@Épgq(a@ŸGù"Õ4?ʹ~%õ²õ?áõ£àðEM@Bþ'Q@ïƒm2?ï½'"ƒ¸‡?˜hÀçCú¿è¢Ë§2ßP¿ëW*ß&Á‹¿î˜ìËoÕ¿ïÿA"VOTHERsppSNR G016.0-00.5?pᘻ="^?q˜fA0{?_±¸S«ê"?e·®W–¿Ë?ïÎcò‡‹>?vùVdXù¥?¹¹dŸ˜µ?·R)Ú6EK?Â3a°ëª?´ÅûvO?èRg˜??ºžÕÞ½?Àþ?¿?¦ºüÄúÓ?ÁŽÌ§õ
D?©Y'QyPk?ç•LrÌë?°Ërz]ùŒ?‰x<¸â¢?tQi~ǤÐ?¶eêg?ž§VX$?ìÍm
@ý™?¡ áðëþ?fNRH­?eqlàn6_?o`7Ó¡íA?w·ù"?ïʃyq°ò?}åñ	ŒC?Ðªy|û? ,NeßE?Ã>ñô4ÖÞ?»ãq5ï?êA¾/l?»«•3r7?·…c®ZƒË?¡í{Ófî?Àš'?)­ñ?©GÌ-.ž?èè®úÍk?°‡c'ü?jMø=ŒP!?[ˆûð†?¿j£tR§?«œMþ
"t?ëøo3OÉÓ?¬Ê0BñuOTHER4FGL J1823.6-2345¿çÜ[ªÏÀ'ÛŸ'xÀ:&Mâ"sÀ;›mB"º?@Ã=¾Q‰à@;Û¾Ø?Îø¾'²!{?Ѓբ‰WW?ü'à@bMÖøtÆ?îøçþ¡f¿ç¼]éÀ#¿áä=Çᬿãù2±-4¿á_Cr¿ïø°ëŶXOTHERsppSNR G008.7-05.0?å+
iݶ¡?½ô¿D£óæ?s~€¢s{?cñõOžµû?Õ]}2Ÿ~O?½ñجÌH»?æIÚi˜u?Á'J§nŒ?üóöÒBÏ?†·<"ÐÌ?ÒEx{x«?À—¿'rP!?éç1çч?«${ú@¯?'T?ôìä`?†ï;¼¸Q?Æ°aBvX?ªRسš?ëJµŽuW?"/Ñ:–?ç¡/×0m?]çá9ˆ?Âç˜q	ƒ?"´Kä,?ÜGÆ{'Šè?ñ~bxŠ?…äžÄ?w†'@"¥ý?á…Ù/©m?ñRA…S?ܦv×w˔?Äzrĺüã?…GÁ'Òô?š­¹ãÆK?áW¥?J:?Äò¹#*?â)·ÏÃ)é?¶æŽŽÕn¨?¥nº?"'Å´:=?Ù	\»þÚw?µq‰ZŸBW?㾦,`Ao?¨Ú0ØLù&? ³ö.sp?yÛ5?ÜÊ«?×x¨hª?¨k÷>ûMIXED4FGL J1824.1-1304?鶚wÔ¼Ÿ¿q™JÞ-näÀ8ÝäLESÀ9'ý÷Cõ@ÁªKÃwä@|5À¬-?Ëó²ª6ÊÂ?èh(=5ët@"£Ÿ¬Ù@i'|'v?ïøʁ˜ñÔ¿Þ1›cHNοç(¬âKº¿ïÿ¨âaßn?èÉâÂW}ë?åÙÑ,­ÝôOTHERsppSNR G018.1-00.1?¥'áédi(?³I¸û¢ê?~Ë©Zr¸?'¥û#bµÌ?îiK†h?´	-56Pq?Ö&[µn~?ЈÓ8KËÛ?­XÛ|Q°?²×øڜÄ?ãDmu×Ñ?Ïkúåcòn?ŞѠÈ?­Ó\]ùÛN?}™*U`?©Ÿøþ4÷ú?åë0år'v?²~ªÝ$8
?¬ƒäÎç¨G?©NS6O?™‡¥éB«?•£mÄ-àÇ?ík"ƒvc?­¸K-ÍY?ŸÿE£€Ö³?«·"ëÚ»?‹›¤EK?˜Ï]½¡Ð?A¥'Ê?°v
ÙtŠr?Àkïûƒ¢?Ç80ь­«?¾ãlBë¯]?ÄO†÷'­£?è–xÁ¡?Ëܙò7ž?ÁŽíE=L?ª8Û!{@?þÃìö°?®úÞW3¤?æÜO"*¢?²R{éS—â?ƒAñ-QŒX?‹Ò&¶1²?¯¡§°Å?³x%`a¿Ž?í¸ÝÀv8}?³ìÅaYÈZOTHER4FGL J1824.5-1351e?Ò0§"ÑU?¿Ý6syÀ6³"÷si"À9N?(3ü@#›Ÿ"X·Ò?û¬	sFHº?¤å¿b%??‹R·ƒ#?öŠÙv0@äÖ¼9ג?֋Ⱦâ(?â6*~®±¯¿Ú³8ÜÀ_׿ØcµÜñ22¿Ùsßà›¿ÌÚeçr~OTHERPWN3FGL J1824.5-1351eHESS J1825-137?qæuž÷TE?nr[-æ?A'l£,è©?C§ÜA5'?ï×ÒyVz'?p+"ѱT¡?§¸üñŽÀP?°áW¨Ü£?© 0ʓ±?¯b{lÜ?ìòh=è)0?¸RÏ7 ­¾?³À³¨¨D?££ž"Ðé?"oÄ- ?À@"ž?ìäkjdÖL?¥ìã*¢º?¥š9œkÌ{?Ž¾lfúmÁ? rê[½Ñ?ŒR$åè|¬?íŸ-À‹(›?—£0…Ô¢?öÅde¿©?w™¸u—NÃ?Fš˜Ò>?D0!>Œûm?ïºkÎÛí?xçD‡˜_
?¤y3QüV?¬œ'gÊ_?©¥s ñؙ?³;93tÃï?í™>?¸´S›¶ê?²«ÑV{5?£Ë»-Q¡?§­¤*¦¤?Š_Ðgd}?í+ý¯mÁO?¥]ÙUðm(?'Ùõ£\pV?'¿!	W?£‡3rj£?–IØ<÷À?î0½Ì0½?š]#3Æ1üOTHER4FGL J1826.2-1450¿ØË«@"¢¿ô¦D¢Ç?ÅÀ6 a3÷À9i£bp7¡@ãR™€@J© öÍ?–\Û£)eT?¿gûfé2@ ¬B 6m@›6PtÀ¿ÖdΡ8Is¿ä ¹ÿȏ¿æ{4ßZÃñ¿è›Ù°
g¿ìwQ­Dq¿ØÇ¿Sg†OTHERHMB3FGL J1826.2-1450LS 5039?wK¢Kâ+?{Uî{H£?xŠ€g†Þ?…|žL‹èº?ï T'd­:?ŒzŽ¦ÀV? ®g/YÍ?°Áº»ve?æâи؜?À÷ÖrµKž?Ð9ê!qiÐ?¿oJûü»'?Éתšâˆ»?­†z$n?ÌÃëŸTR?±#¤@ñʤ?âYqˆ½?³×û¾¢ž˜?…Œ<©gI?plW"Ç?Їt±Å?µbÑÕx­?çfƒ~`?µîQ	"ŒŸ?d.¾ô
î?b¥ñã§ð¢?€òIIN?"ü#ì21š?ï©ßRx¸?†ƒ¶WÀ?Œkm¸õg?•Þà3z?ç¸QÔo>¸?Åoy¢$Ïå?Ï^qöù'I?ÅÊ"9?Ǭˆ`ف?®%÷gSl?Ïi^ñۂ¦?³†ÿ£$O?â:†*ÉNµ?¶…{Ç¥W?k ™Ñ?}º?Z«!º6à?Ó^"ò%ø?Àº"w,?æ5&>?À škóædMIXED4FGL J1828.0-1133?ÚOqèOµ¿ÂfS†ÑšÀ8Nµ‡5éÇÀ9îÐ_(""@&Þ÷q@ö¥†6æF?Ä/fÉû?âtöL"'@'5Ÿôým@eãmx(†?â ÀaŠ	?ԋ"|I&º¿Üi'ûr}¿êfs.ËÅ¿îrç;
¿ŸzSƒ4ÓFOTHERspp3FGL J1828.4-1121SNR G020.0-00.2?Œ:ªÎÜX?M}åð?¾ô(A£Ë?Àù	ªw¨?ëËy@×æ?ÁU"¾àÈO?±x;˜'?¯ßüCKÈð?Ñí£'Àk?¼ÿ±![Ö|?äÚ-/Z'û?½4±&lë?¹ª°BRŠç?¥{ÿÇú>Æ?ÏBŽ ?±ç9þ-?äúw?³Ýî¥"h?ïþW†?v6MA@Úî?ÃLA÷ò…?£#wë~P®?ê¥o';ë?¤ý·ØVæ?|Ž'ô?t«Ätz¯€?Ìô¼Ú*G@?ċÄs%ÖB?艴z¬ªª?Ğl>d:?'üì¹ÌöÛ?"ýWAþû?Ó_`äµæ?ôðo
Ç&?åÀhY?îVRƒA?­Ð—I‰?™£³U£?Ñ3ÄÞ@è~?¶·#Ã(´)?å‰ׯ²h?·._D<?r14š*Qý?_ï4Cê±?È)Ôz@7þ?²ÖÎ@Ì@?éÑ(x]ùt?³À{kíJOTHER4FGL J1829.4-1256?ïë¨Ó{ñ¿ñeªIFÀ9cQ³PúÄÀ;ƒ:=°@¼]¸ÂÔ¦@"¯ûî|?ÍÛ`#`"?ïÛ}i¸*~@õo›Ìz@³ɝÃJ?ïƒ{_œÈ£?ïÚËB‰Œ?ˆ¢õ¸ÔG¿è¹"8à¿ïþ>>ª	Ô?ï¨wÆOOTHERspp3FGL J1829.7-1304SNR G018.9-01.1?¤ÐqÅZ¶²?¤eû£Î™?Ǹ)|¦Ù?ÂNè½»"G?èÄî"án?ÃqTZdj?©™Š¾?´ÐO"È©?ät†^©?Ç'à}Èq?Ó÷(zq-?ÄrÑ«?ÅÀÏÀ"|œ?ª
QŸ gì?ډã0ïê'?´`g"{Ü÷?ڕ´ïØ·ß?´ |[]…?¢¦¾@ÿ	ò?ŠŽ¹Ùºwß?ê÷sÙãÙ?«AÝøœž?¾ôm>‹šÂ?§§¥"ÝCÔ?–:²&¯÷g?™-eÏù¹%?ÑÑ÷'úòX?ǪM.I?æe.¥Ú'n?Çùc<{?ÀąõZ²?›åÐF,sÌ?åTµ@?ËÑ@jåbV?ÔËPq˜¯Ë?Ëh¤ŠŸ'ç?ºHEìÉA?¢ÁyônÅ?ÛWU14ÖK?º6Ùt¿´O?Þ¤ýO÷d?¹†kjaf°?~Ìç\—›î?qU$80Uƒ?ìd6‰»s?«":[_?ºñ}=9é¨?ªp³T'_ðMIXED4FGL J1829.5+4845¿Ñ³.Áž@7Š\å´$À8¾©@'À;ûl'à±@B˜*Þ@ÙuòËd?¡òœ*'?¯'öiÿ"5@êeÀN9@ë財*¿ÄI'C¼˜¿âßwßµ‡·¿ç›˜w[¿ã".ülοë€JœÜD¿ÞU3ÃÑÑnOTHERcss3FGL J1829.6+48443C 380?ïÈ8$"Ž?«Œ0¸J,÷?q[̬°ë?«—n‰/?e¬-æhb?_eØć?ïÁR\n?'+ìžuŠ¿?`@[ÃRÙ?pE¯~áœ
?wQ(ô6dh?xÃĜîy?ï}­A¹?ŒA,íŠ6Ä?€'öCÛx?……•.9Ÿ?€',ÒÃÊ+?€CuxAû?ïÑzš­b?UC
ISUô?dƒ\ÃÞ"?H½Ýo¬7?jˆÁë'm?J
ÿ}Å?ïÅÓˆ¹M?r…Ba[à?ZèԇÁ?S­=*üڑ?v\våmå,?oM|çZW?ïv띃š:?"à&ÏUF?nƒ7½é}…?€a$Ù6f;?Š¤J®—0?'³‹ù—?ïw5¯B?‰ûBR¡?{€î+·Ø?"š‹@—H&?"rß«?@±ö-«v?ïdóRP8?vÁÚÙj>?{%‰LP'Ó?læ?#QIç?~'ýv]_?gê0£ŸvAGN4FGL J1830.2-1005¿ìصú.&?«W2"Ç{À7×)ž^û8À9""išÎ@¢ÌÉè>@
Å㤀?ÄA¼bò= ?Ûæ€<¦N‰@ÓÖ¿•?ôÈ[á¨&$?ï±½¢bk¿ßZ¿žæàt¿è˜8p‰Õ׿옝?ìT'¿ç?Ô@ßn:¿ïÿ·ÀÌ
ŠOTHERspp1FGL J1829.6-1006cSNR G021.5-00.1?‰á3©S4«? ŸábT4À?«Få	$?¶­û‡g–Q?íçÃNÚë?¸X«ÞWÉ?¦Bkm%?«2ºôV?Ê%7œúL7?¾9¬w ?è‹gŸ?¾í€®]˜Y?¼ÓIÃ|?¨¥xÛâS?ÂÉÞ®ª*"?¬¥'¦¦
?ç³1ýØ?±w\ vº?lŒ  
<?VÄ='¤D?Áøºøu?¤øY/«›?뢭"ÈN?¥
{SêU!?'¿f¨Èb?†³;íq&?°bnûòet?»Þy
?í¨µÂÞÑ ?»ßj\oí?I±»(©?—IªIéMÏ?Ë«<?‡'?Á·>4u?èŽúãÐ8V?Áh½49©«?¸X‰dÏ?£ßa).°>?'çrYR›?­ïì¼ <ž?èP4ót"ß?±ëWÖë/?JyJa¼.ë?<Ö5A3?ÇÁµ%Cå?³'õ;•}?ê	@&?³òÍE NOTHER4FGL J1831.8-1503?¥Ô"HJ<QÀÈõÝgNÄÀ:™ °åºÀ<RG—nF/@ÐõLrÊM@Ê}Å'¼Ý?Õ8¥ƒ1Î.?ïý'ÒÕûJ@ÃC·õf?ü€Ó6ô2í¿µL+@V?ê?ýkûý?ä`s^™¿åª%mwҟ¿ï$X*Ž¿½pc×%ÁOTHERsppSNR G017.4-02.3	?Ó
Ѷ|ºw?À³ÓÝY¯?Âdµ¹WF…?¶Ñ‡3Êä"?áái¶kÑ#?ÃwäTË*Ù?¼-¥LR?¾ƒp€y?»?ÔʉÎAäH?ÉBu£ù¢v?âuÌ2?ƁºÜ®¾?äQW‡À!?°Æ.t/óP?Áš…×è?§ê"°g­?Í ¡ÖT
?¬'q¶^rè?Ñ/»[­)?±Cà—w?â´îE˜?·Gl¯ ?ŝµ£¯P?¨uJù•±?ÅÚ&$Š?¶»S¸'Ëž?ÉnÿS?¾ÇqÄ4ð?ä-ó6)<?Âø(¿«•ß?©¬½_\á÷?±jéÄ.Œ"?ÑÓÒ×ö?Ì#ž¤µm?å{J¾aœu?Ëôñþy[û?ÜIØ"'?µ¬Ô¿{…?Éà†'¡Ú†?²[§j™z0?ÖÆ l–?´>Çq0Sa?¼Ð_5gv?¨
ÊÂÞÝ?åxuë??½Œ?höŽ'?Íiî"ŽD?¶KNÖÁ‡MIXED4FGL J1832.3-1433?à™Ñ'¯D§À¼,†pÇéÀ9ÌEŠMÌ<À;=5¾(@]l²ŒÛ?ÿSýÈîû?ЉCá`x?ÙmR=åhÐ@ø£ë,3@À<-'Å¿ïxvétù?ì®ç¸5f?ÒP×Þά÷¿çŽáDS(¿á4&¾Ýà¿ï÷åê«%OTHERsppSNR G017.8-02.6?áq)ž'…\?À‹÷Z™?€éáS@©?s²o¶i²?ܖ]¸J'S?Ào\äÝdË?äÖôÜ
'e?Äy×ٝñ?ƒÎ×︰›?…—;#Gw?Õ³Ÿˆà¨'?ÄƤŒY?àó@·UAP?² ¹ÖGl?´¯³2-4þ?¡eÀ)I|*?Øí'ÄÊ0!?²3m<YÒ£?â[–ñ•üN?²_&垵?–/1Õ.(?{æÊG¶öÀ?Ùåàš	+"?²¬Èl…?ÒaݹØY?ºO¾¯'Ë?–[Wà®Ú?Š*Ìe?æ88'Ó
?»€6F8©?׏¤Í:ù?Ç
Ól¾?‹ùOhœAW?•$]FEù?ãÈH[c}ÿ?ÆÖ(sÅ'E?Ô;z:¿Ö?²¾9U	?ºk¤Á:?¢''fQb?â°íªxÔ?³Wµù'œó?Ù/®Sõ?·ÞeÖ$Ÿ?—'pý»?ˆOHqñ¥m?⯨Ié5Â?¸½oq-èçMIXED4FGL J1832.9-0913¿éì'£lg¿ÁÁ›o¨ÚÀ8Ó^R›®GÀ:†••þÚf@h'Ô±Ã@û]‰H¾?Ìwt«£‡Y?å·Y}ʱ@Q['—@¶HW²™p¿ã€üŸxUÒ¿×xû~æåÓ¿Ôîÿ&¼,l¿çXUÌ»/¿î–÷'ê)Õ¿ïë;³´MOTHERsppSNR G022.7-00.2?¥eÝÙºq? {P"¤?ÐQþ"3íÝ?Ã?b$7?怯øM%š?Äï:ŠëV?£Æy˜­?§À²û#ÿ?ȔŒKKÐ?¸ç'F3ú?èžufçô#?¹üîEËï¶?½.¬÷Öw?¤Ö|©íÑ_?ЈTÝÒف?°íÄú¿{
?äÿò¥4¿?²7¾sÐn?§È~Ý¡Ht?†k1EUQ?Ã;4åÌh?¡k€Ç.µó?鴪ؗl?£¦wµ?™k5¯Ä'?Û=§ -?˧GþhÉ?Á+§õŸK?èMˆÔ¥^I?Á²o"ÙTV?"­W²0¤?•Óß^Ìst?Èú÷«
?Á$‰º?é)f—IïI?ÀÐ"*)ý³?°È€$*¯?ÞiP}PK?Ñ»-w a¹?µ'He•?å	Y?·P?µàýW'h"?ˆƒ
nÀhk?q&h«y'?ÆpûUK`ü?ªvc^Ÿ»?êµ)ß?ªù¦à*ØOTHER4FGL J1834.1-0706e?ìâ
?âºíÜçÍÀ7‡†Nc:bÀ9÷‡©­
@ ºÓ»ÔW@B¤¸±?ª6CM1·?´¯Ï;#@½M%LÀ£?þ8r_˜ìË¿ï}1NV¥(?ïO¼5¥Ô:¿Ø_~Øտܳ@S'D¿ä…|áÒîO¿ä˜…2ˆKOTHERSNR3FGL J1833.9-0711SNR G024.7+00.6?¤)lÓ‰+?šÀÇÇ?"©8Ú"\?"@àf¥Úÿ?îjÄR'­?žˆÌ|KÔ5?³F"Õ?¶2dZ˜Ó?Á[PŠÔQH?½ÕRq*ÔY?é@iÛ¢
î?ÁÉs¾•õ?®]-o´IÇ?¡(x×?²3jŒºÞ?¢}ýú•Þ?ëÓ¿×_¼˜?ªîþî
žº?µoQâé"?ó6ÉÖ?³0GΑA2?—§·1¿ ?êìÉù?§†È1û?ª$ÿZÏÁ?ž>$—¨Âp?†MC±ƒæÂ?"Dƒ_«?î‰?¡°é×ʁÄ?¥]@¢Ýe ?¦"ÈkÞQ?É¢FPò5è?É%Ò	^?èAša•œ4?ÉM\ÆÕq?°º@]\4[? 69:Û?°?Ô€?£ƒ…ÇYå1?ëæ¯ùú¤Ä?«?æ$*ºe?¥»¥–©¯y?"
n̓ l?·Š.*îg¾?¥#6ϕ—?ë²ÿán'Ð?¬¹Ì±GUíOTHER4FGL J1834.5-0846e¿ÖÞ˜•/¿ÑêÛá<ÆZÀ6øêúÀ9´ëvÛÿp@!q3­ª@øã["‹?©ãZ> 2a?¡7ßÀD~4?ö˜ÏTf‰¢?ðX#…@FA?ê!j³Ó¿×AIÌR¿Þ|cÓº¿ßü
1¿åèå1G ©¿Ö¿²ÝãJ"OTHERspp3FGL J1834.5-0841W 41?"=Æù½àe?§Ί8¾è?‡D"4¿?¯Iø+&H?îÿÜ·¯ú?³Š("Ð×?‹}x¨g¦?™ Örë?Ê`i"'˲?Ę>Û]o?èû¥|¦Å?įØ µO?žSàŸ4?•]Kûû`?«$ó]èåó?¡ŒÊø8×?í\Þ+*6q?¤–\¬¶ÿF?ŠlYügón?t\ç"ß?¶ÞK™>Q‹? R‡öÔ¿'?캅$Ë!?¡ˆ.ÞËä?†]Ö°Š?µ"9;§"?~—ô'1p
?€wôÅB¡‡?î֝(y¤?µÊ;?"öSõ"?'9½è°s?ÄÐñr|&ö?Ãd¸(v%?êwë)ëG?ÃuË|e?¡B=ïró?•(zD*+—?¤w"ѬÑ?¬"•þšÕ?í¤bñow?¢ÐA|p?¸?t»mÜ«Ø?ep¸Ù¸G?»ò""nƒä?¦iÕ"/•?ìY…öà­»?¦ÁRX-ÓOTHER4FGL J1835.7-3258?"QìÙH
zÀ&¼q'êRðÀ:"¾@BÀ<#=,±8ó@³7ƒ$O@Ê#9Àëî?À‹ön?×ÍýNtØ@R° ě¦@J~}"N?ïÿ?`h¤¿Ã—Ëù")h¿ãmß âM½¿äQQ¿î;Äf̽³¿ïûç6Û^`OTHERglc3FGL J1835.7-3258NGC 6652?Ñë&W`A½?Àþg4]?áÑãž0¾?Ä®u'Ûè?ŲkÂƹ?µ9'Ao?Ú^ˆ6íg?Çî°6éöÿ?Öµ¹95ðl?Ç+'s7Z?Í×}!`D[?À0?\{ë?Õ1%¡û?´y}DyW?à_IÜ9s¶?´âêËh?Ä HþK ?§äÝ$Þ²?ãVµfÝ7\?¡›¿K `Š?ÎwKÈͱ?ž'9@w ?Ä-ޛ½qv?–ULˆzՍ?¾÷¼'°Q ?³	î¦/aê?æÍIÁ·g?Â6ùf]×÷?È@엠ù"?ºýÅcÞ?Î@rî¬gõ?ÄÓÌEhj?á$Ã}\é?Éç­´ë?Í,áTf?ÂÿZïöÙ¢?Å7›ë¶û]?­½JêE?åAG
¬?´evlyî?ÅÃG¤­ó?ªFa"Ú u?ÒŧLI?£'2w3ƒ´?Ûò­lgæ?¬})€¿É}?ÑHTDGO?¤!µê)¡[MIXED4FGL J1836.1+1143¿äSkî¡Äò@!\^Ô¡­dÀ:uOøÃÌÀ;ôWVP@Iބ…5_@Úµ€í ?Í°£vg:?Ð#Ëâ5!@­Ácâþ?út"« «¿ë¥C¡?€I?ïôἩi¿ÝCm¨z-¿çrº'Gm}¿Ý‰šÈïÿð ¼x—OTHERunk87GB 183342.2+114143?èb§ÓÕ:ì?¸´VõøB±?v{hs_]?{üÆ©¸ò?Ìf'D
›å?·þñ×̚?èÄá'f?ÃϒQKb?©Î{	Ìâ?©Ã¹:º4F?ÆxÜ )€­?Á#oÞV¯\?ë1¤F-?¥€Íô(×? ¾‹!¤?å—…("•?¾nÎûâJI?£ZM"Ü–C?è&«;"»?/‹G—$g?©ÙK;`Õã?ŒSšÞ?ÈïB3ðâ?˜ƒ`$áip?à
MÊç?Àvü-/?£ýɀ"`c?—Wb½dyý?ÝB,4ç=f?À6'óåÀ?á±±kë?Ë«Å9Ê?î?¿ÇÃEÞ?½È6>o@D?Ôª­)楳?É°s'?åP÷œâ¬ç?®0›a?±¶wÿH¨™?›40¤±§b?ÐðrÆh|
?¬ò-ҝ²ˆ?à‡Áy)?¨·_Ÿš1?µºßnÍً? S(Gêã?ك µJX?§­¦ÁË;þAGN4FGL J1836.5-0651e?ïÿúr]¦µ?ÄCO¢ÝÀ6A‹sf)*À9"Â(.s@!&¤†‡™@;ÌDÑ	?›2Gk'í?Œ8e!Aï?ñ8^€¾×A@9nY$¿áµþŸWɖ¿–¦…Üàc¿àÔ*ÄϨI¿áÖG4q÷"¿âÃai&Š¿ØuØstOTHERpwn3FGL J1836.5-0655eHESS J1837-069?YÏ.oã?­XÏï©â
?Q¿hœݧ?[MtÝä€?ïzÂäk¤ê?­e²Æÿ?¸© ŸÜ«?Á;M!à"D?¹¦˜¬Dþ?¼ÅB)p;Ò?é¶Öú^g?ÅîGJ0>¦?°ªÜ7þèá?£*…Èà?¢ÁÈ6åð4?™´È¡€)?쾇õ­@À?§ü]•#Á?º¼–‹¥Ä?¤±|âš7¦?±^¾fÖ?œ,¾œ'?ê|¨	sò?¬³2u\É;?—'ÀŠàsg?µJDf'?ZÒ½ˆQiÊ?e'C`*ν?ï9XOP?µdŽ:?´b®«6•Œ?»»Ïµ›"?¼}º;¶Ë•?Ã*}³p@–?éãòãYMœ?ÆÁ¥ií–?²@ÒÒýØ?¡òR¶cÝS?žS3 ï¸Û?•EsײÛ?ìÅL}c>?¥ËæO?­ëf!êWï? ¡ä4mQ?¶ït#ŠÁ?ª'_çØR"?ëC[+J1?±ö""ºmOTHER4FGL J1836.8-0727?ìF6ߞO¿Æ¡)ÛƏÇÀ83È-*ÛvÀ9õ}å-@¥ˆáe‹@8ƒŸ\Q:?ĆÒíx=ÿ?ÞYG™ò"í@I[»èxû?õŒ>Ù.°¿Þ†=0âöÛ?ájÅÁ?Ðпáµ'ÿùJ¿ê½®ˆ*Ü¿ëleöÕ¿ïÿð°×£ÀOTHERunk0FGL J1836.1-0727NVSS J183652-072453?"òÝÖÕý?˜˜åçæ*?Ò¼€æ碈?É*\՘ù6?æ7õ¹œ?ÉhŸ¤~,´?Ÿ?â
z?¡ìV㎻?ß¼Šõ¼Û?Ãl[Ü'fT?ÞOvê[í«?ÂÝßÇs?¹ƒµ‹ã?§CÖ…!*?Ñ×åè…B¨?³0FÃk¡¥?ãã–Ztë?´|^æ¹^»?vjG×8?YI¤a?ÓvÂô»Ì?«c()¥üå?æ_±&º:?«­¿ÃßDG?}g=3a¶9?wœ"ÅÒ63?ؔ¿éx]?ƺW4b'?ãzÑ÷r×}?ƺ*ü¶}?'M@>xOŒ?ÿ¦¨p®?áëˆ W ?Ç{O÷ºT?ۖ…½ïE?Ç;lÛ©9?­Ô[Cjx? ¢Lµ?Õ`±èè-É?¸4ta1æZ?ãraWš?¸øòHÇ?V=i÷yK?B8p¤F?ÖÛ%.?´Ø9˜<=?ä‡NT$s?´äKö¹àUMIXED4FGL J1837.6-2904?âKý¼PJ=À$"¹,HÀ: š=-‡ùÀ;ÞËêN½Ó@¢Câ-@Qš&‡S?ÌÇ`|B?ÝÙoØ2@4f'ëØ+@	…nVŸÉß?âó\²¿Þ¼l—ØÏ:¿äJ½"s嫿薣L;¿ã%žÀJ‹¿ïÿ-<y-OTHERNOVV5668 Sgr?ïmeÑ*C?‡FX¨-s:?"KP'¹?3èøïñ?€%t8?tžTOF¾ó?çZDS¹\û?DZý¤Â'é?§¡"âɇu?­¯äғe?Ì®¥øÖ·?ľ²€£Üò?êZ{îÛ7?¬:ʗ?,?³Ãw.LÓõ?¢'öˆÐ!*?»q´ôÐP?£Ž%£5}?êDmñ•? ÙuŒNK?°.ïÀ·?¼¯…1ë?½]hU;`? Ôƞèì?îÜz¯ž"©?™\»b">?'§xœ¢LA?Ô/Ã?'É1mÓp•?‹pÛ'|?à¢{%ÌT?Í¡Hs¦Ï?Àó˜Óöâ ?ÀWbû«e'?×dö	?Ë
"
Ðò?çêõ¯ø‰G?°&òià?»ŽôÏö"?¦á7CâM«?Œ®Ø"Éâ?¨âm_3T1?ÝØUÖeÈ?²Z'Q¦¯º?ËÆ4b\?±q^Ìj?ÔDø—<-?¶oϳcAGN4FGL J1838.3-2148?êÂú¥fñÀ‹;26À:h Ä0FÀ;딾h…û@Tñ¡˜kœ?ûžƒ
f?×µ˜ñ/?îªâ+Ù¢ž@&ó|cþ­?óZ…tɀ'¿éK—¾":?ïÝIúÑÿå#flE£x¿Ù££Þ–ú¿åñ0ߛÜj¿ïâÁáaYaOTHERunk1RXS J183818.2-214857?âÚ%Vëbÿ?ÅtÅNÔ#ƒ?‹._" ?‰Tó6í‹?Ùo;ßK¡á?ÅSò¨K®?ÑvjŒÞÄ?Æ×)ÃP€?Ç)ÒÌÁS?Á£×çnIñ?ázV`±
?ĕ7Hš?è‰ópz*?¬®©GÍÏ?°Ø%z]Ë*?ŸÕɞå é?Ål!´?§Å-ZÑé´?ÔÜcNj,?¯Â™âҎ&?Ò©Ñ	ÈUÅ?·ûbo2~?Øz'é@?³ÿÀŸÂÓz?ÙÔP¨þ«0?Äۈ«¤wÞ?Ÿî—DL,¡?™í®3ÕQ?âbñÓ?Å_HUëU4?¾è­;?Àz«?Ð7q-ñ?ʆ¡v²?ä1Ε`
?Ë­¹â}q?ãÞC,%?±•žö$à?¸(;~vº?¥=µË±ø?Ò9Æ!"V‰?°	1›"?ÅUö}[† ?«.7Ì¥(§?Ô E$ï›?Á€¹+Õõ?àZ|¾¦‹?ÀºÕ*¶¯KMIXED4FGL J1838.9-0704e?ïÜDU‰8<¿Ý¿í@_Á‡À7c½ZiÀ:
²p*4‡@"EÑ4O?ýTç4?ª­ƒö?ž%.§w§?õ-ÑD*Ò<@SÖK¦¿äWLíï\D?ìÛÊ`áÂ'¿Òé,êCÖ¿ß4<Kµ¶¿ÜÔ–j:¿Î¿r[½OTHERpwn3FGL J1838.9-0646HESS J1837-069?§»ŸÎú?¢…VÖ iŸ?e'êy'?nÌâŠcòŸ?îz\[0ä`?£LóU{O?Ñ^NѦ?Ì×ÕryÂ?š¢.óÆQ?›AÃU
û?æÚnë-?ÌÈA°@>?¿9oýâ?¨˜ûøª
j?«.y¼¹Â?¡Wù½K?êeêd¯¤j?¯=‹ä•º?ÑÄ9‰þ4é?®ê¹F#ä?GÛÈZ?ƒËȳR?æ3«+ùiI?°ÁjIô?§ÂF!|›?¨ÈmfD?f&dž9/?keêh‡´…?îx}RÈO?©r˜¾:S?Í ãi5<'?ǽ,ԐT?'"V¬>:?ŸÁó0âìŒ?è$uˆËÊ?Ç׺y숲?ºuD®8k?®s÷JY'?¢ø^Zb?œi÷‡¹ÜÖ?ê!ÜÍå•_?±î×Ê?Ã׿ÞÁ…¶?«iYÑPÂ?¡Ô3»œ¸X?'wDÒd]Å?éìÌÌÌÌÍ?¯€ÕޒOTHER4FGL J1839.4-0553?צ$N`W¦¿›8g®´À7Eõ­–§À9T'œýÒ(@c;'PŸÖ@Ð:?–îÄ?¯RSÈ)$?ՖBÚ¶@(dÀ
¡©@Ë#œè-¦¿ØœOAÙ´?¢b`¿ªÇ·¿áÈÖ"‹ñ¿å¼žK°»¿ì'ê@%4¿ïÿôým~‰OTHERunk3FGL J1839.3-0552NVSS J183922-055321?¦Oz+^5g?ÀCªú•?è{Ü`ØKË?ÆÓÕa{Ï?È|¯ñþ=;?Áº4}ÏÓV?†¨Ì²'X?šúñUûÝ?åè¸Cäíf?ÅÉ´XP'Ù?ÓyIçŠá?ÅcéK*M?¦ä‰¸:? 4s%Ø?骃RÊ(?±±ÿ-¿xH?ÜÐGx?®î·ƒ9…Þ?WHíraô?E4›,Ø?Ïp²êp?« ãW+I«?è.ΰ¸Ö?«›¨Õ†5¸?§Š«VdÎ|?È#9aÊ?åëL¸¦‹V?ËXwMÇç"?Ñ8#"Øå?Æ=–¡Ë?w†¿)§•?…šÓ,AºP?è¬"5ŒÝ?ÅÕöóqÊ?ÎÕA¹;~?ÅÙ-Ÿ0Ã?¡_Â~ÝY!?œó{Ð?yç?ê€fÈ?±vñV¢¨?Á¦t?å?­?¯?*/¥öN?0q'}s?$ù–)"¹?ÔåEûž?´À¥Û,?åóÿ8&Y}?´Ài´qÄMIXED4FGL J1840.0-0341¿ïêIò‰Â.?ëXéÀ9iS$jB"À;?Ú˓é@ŸAЄè2@Š…) ?ÌÖßuEý:?êù¬ÿ§ël@Œý©äj@'bˆ‹T\¿Öüz$r뿧Š
¿Ó‹‰ þé¿å»;u!M¿ïúøÞ£¿ïÍQ!ZÛOTHERspp2FGL J1839.7-0334cSNR G028.8+01.5?©_\aùÆà?¡·KŒ>"ï?ӉyÒBÇ?Åþ¬K€?ä¥{|Îß?Æhy]†eW?–ôØè5ŸN?¡%㽟ËF?×&Î;óÝC?Å6|Çð?ã´òퟴ?Äå,ï;%Š?ÂçFçkè?¦nJ,ì>¤?×IïbMýå?µ%8ü¼LÏ?ßBm">L'?³ä#•+Vã?­ôK"_K?ŠD&
Z(?àj} ßk?°¦Æ+\ ?Ûl|^ºs?¯ŸÒò?'¼{µœÉ>?…¶Œ"öj¤?ÕÿÆ*,Š‰?ÅÈÉÝÚW?är9
<Ôr?Ő܏@-?ˆñ¢–®²Ï?•v
7T?×ÀK¼¨#?Êy'µq2ë?ã¼,Ïtz"?Ê}®CA?³?±Ð*";+†?˜[ŸQÙ*m?×,OZA{1?¾Ò^NjšR?â/Ó\`?¾2½UÔ.?‰Âœñ]'è?uƒLúOT?ãd¸|Þ£?µ¿S"ºÎî?Øi­¦Ÿo$?µV?þåÒMIXED4FGL J1840.0-0411¿íÍ
Ãü³^?ã²â`1îåÀ8Ë6Z/ À:¯X¶zzð@§qºGº@Â…îÁê?ÀéÁЈg?ÕTpšœÏ@T´:ç?û£gΛY¿ëDä þè©?îAÔKFOp¿Öç¨ñ%r¿äd˜0
¿ìÿ"=ßßy¿æ°Ë¡ÖªOTHERspp3FGL J1840.1-0412SNR G027.8+00.6?—š›G$Éç?Š:‡±=?׳ӈ#?ÅYáåéÔ?ãiAa–•P?ňs{±B?"'\LmR$?ž&—ê#+?ÓZ.Ýìe?ÀíjbZ¤M?å®Õ®¦N¼?Á͂ÝÈü?¸4üžè;?¡SC69?Ճϸp¨?±_Á+!úx?â7xÞtPE?²œJG΀?«µPÜd?…躁*=ê?Ï|nÈW°?£ø6´§Nÿ?æeLŸÑþ?¥)Úhó‡Â?•U•ìb¬?‡vŸœýw?ßmοɸ?Çyþîµ?ß=¤ÒCŽ?ÇflT‡?…$íHûe?‰†Á§_ú?Ö'GI7"ù?Æp×zóÁ?ä—ȦûF?Ædpïùš?±éÕЏK£?™ÊoÉhH§?Չ©`zØÓ?¶a÷út''?âýð•Ì'?µÕóx?'ÍmYëEî?s<`"½?Ò¤ûâ0"?±³sxÊK{?扗1Ï?±ÙŸ"ðoêMIXED4FGL J1840.8-0453e¿ã܈.b>?¿¹Ÿ'À7Y…tH§9À9'$~d@ˆ¾)pçŸ@úh±šA_?³uÏ:p`?Ð4°@¥¾@	G{À?ütXåIpa?îfKŽs˪¿ËOøæ±${¿áç—Sn¿çá}ÿ	_û¿é¹Ù«¡¿áĖgµñ¿OTHERspp2FGL J1841.2-0459cKes 73?{"¬³Á?tÔ@*Û?ÄÄ ×?ÂKP‰t!?êÃo
œ3?Âf:d0è?ú²K1Ñ?"¬ºñs™W?՞}
Ý
?¿Úäp5%?ä´Y†Y ?¿r¹ÓBT0?®WAìo¼?ŸÂÖcUc*?ÎøJÎt0˜?³@/Â
Ì´?æaØD,Þ?´9¥"/ç?uSÐÊxر?_y'B@?¿ÔÖÆöŸ? <`m"ú?ëÚ½…~{þ? æi¹
¶?v4Ï|iÜâ?q·!
Njì?În!›± õ?ÃÙw†a?è8
ùùçÉ?Ãü…ÊãF??lÛÿD?"-†8"b)?Õ[
4úfA?ÄGý³Û ?åÇ^Mé?Äe·_'WÞ?¥ç4vèZ?™7Û¨K§ã?ÒoÞò`§'?·óRïe%?åi?7ðª?¸ÌNpÓ5?Uôæ1ÒÔÜ?Cò샩59?ï‡,.²?©wàï7?ë	#Á¿í/?©¦‡±Ã9¯OTHER4FGL J1840.9-0532e¿·@|ûÊ¿Éc\ɯŒÀ6ÁHO$*'À9¢ö{@!À¤¿:¾?ÿžá¢FçE?¢qNCQZÞ?~¢¨¿"?Þóå÷1?þ8=ägF?çÞ&'dA¿¹j"Þ|L­¿ÛO
*á¿ààÙÿ»6¢¿ãäkß÷÷É¿ÓKA\k»»OTHERPWN3FGL J1840.9-0532eHESS J1841-055?t1õ@z?k$£Ñh`?Vp]ØÇ°š?Yçé‰"–?ïÌcæ"Xë?qmNFèÒ?£	…²(~?¬;¢KóZ?µiÏÁ¥¥Œ?·ªwΝÑ?ì"-¬¶Ý?»ÌC$—ää?¡¿?ÞE?™}iƒèˆ?ŒQCÔ?‡›Ž1Bß?î~?y€'?œˆ¿µ?Åñ?§ÀÎOêà?'NªÜÛS?¨É»¥|·?"ÙPÖÁŸ?ì÷[HÐÿ7?ž©Å´ö.?q€µlê×?z'où=R?Z¸9E²˜ï?Y<™PÓl?ï¬ÝàŠ2¸?}¼é"hÐ?š=X´?¡u>'9å?®Bé5ÿ?µ³B…Ë+n?íJößM‹'?·ruNœ×?žt¶¶5Æ?"‰±mk€f?‡œ²¬Ú?
	Wì?î®[ׅý?–œ%B¸>ÿ?–~Ž?å>?ˆŠ³Ëꑾ?¬ªµ4ù´?™èÝe3Q?í`ÆÐo«? 
bJOTHER4FGL J1842.2-0751?ï(R¿•²¿ø֍
?#À9m‹U38<À:í‹ÿ}#@an"B€@]™`Ž¶?ÐL]їb?Öļµ'•?ý*áU
È?û¢£h¥Zî¿ïúHÿÏ?ïÏف¼O¿»³¦
@JÉ¿åÛêaˆ0;¿ìXG¢'v¿ÇF£¨f;OTHERsppSNR G025.1-02.3	?¼"Gý˜š?·&\ܶ
$?"™¢›#q?Žb߁Â?ëÒ©ë¡ND?¸¢Ù~‹÷?Ò+*Çe?"èDÓ?°‹–ðž˜?¥'['ºe?äÚy)¦[c?Áÿ'p*_z?ЎÝ$Ö¡?¯4—ø‰Ýó?Àd³×Õ·?§Ó9R¥÷ó?㟊ÀžýB?±Õštt–â?Óí՝Î?ª»Òzé»?¸ûq㸚½?–Žä†h>¢?ãP›=U?­íÑët̓?°¯<Y|¼ø?¨ËRE¿tA?FTY:Ý5?—ý'û ™?ìÿåÒ=‹7?¯G–†??¼¿.cž>?·
Ñw8?´_Y·a?´ ê"(³ ?éÜ2bþ§æ?¾™¨·]"ž?ÂæQqü`}?¥êò*,?¿¾¼mý¬?¦Ñ#(çs?çN"f¸‹?°\®+^îò?Âg;ãÛÝ?¤ Y"ß+?»øqì+?¢ð‡m\u?è1ùTó«?®n™'mnOTHER4FGL J1842.5-0359c¿ïÚ¢ÄPâ?Ãå>]³ºWÀ8
°Úþ¾·À9Ÿ»	Uê@Ýp3Ü@jZaueÞ?ÄèÀHZå?؅ZZna@\äŒ×ê@‰Ö€TÏ?åi¹×ý'w¿á<Ó$Õ¢^¿å€™¸£J¿ê?*b{ö¿ïþmž"ÿQ?ït4à‡iÁOTHERunk3FGL J1843.0-0359cNVSS J184240-035858<?¬³Ý4†6?´Ô~ž2Þä?…|+•G3ø?'"÷gbâ9?íÞÑ~"·­?·tÄyÌ?´e?îÚ?µÙüï»W?À!yŽ°\?µ'¤bïe2?évôçPº5?¾"0ô¿…?ŸÞhfØ?«ù՟}`?ÅþüÕ~!C?­´Ú–þ£x?åϘÓ]ù?³ñ¸~Ÿç?'u¿ÏØ'Æ?}8'¨×Jb?«˜Û ?áöÛ?íºÈ#«çá?•I³t®u?¢lšV.À?¾}"èn?—ÜÝÒ]ÏL?¢d>µÏ.?îOkÅmT?¿þ5`Æ$£?¡½Þó?þ?©S£å#»?Á÷Æ?êћ?¾ž;C;ظ?êf0€ÑK¸?ÀR)5 b?¸áu™gÎ#?¤±ˆrŸ?Åéœ)&??°\þÐklÿ?çijF¼¬?³'>"R¾?l1»7›Ç?`RmBž9?±ÑQ	¦Å? ™ÇØ¥j?í©¤#`WY?¡¶µOTHER4FGL J1844.4-0306¿Ý‹ù÷
9?À0¸@¸À7±Ÿ°4ÒÀ9zh»«<Y@KŸÅÒ=@K9âyÝ<?¼@|ÇÑ»I?ԗ?a¿¸'@7?tN†@k%ПX?ï%)œ±|¿â0öýø¾Ã¿å'0^—ÿ¿ê–—†™ã¿íïßáÒmv¿ïöÁ'ÜæöOTHERunk1FGL J1844.3-0309cNVSS J184431-030716?†@?ÛïÛ?"wK–ta?Ñ"í•ø®?È
Þ
6åš?ç$4‰ŽMz?È(†ÜӀ?¡œCG^?ª¼^³@_?Ò}äŽ×Á?¾î Wß÷?å§L"G ?ÀbQŠG}S?¯ÿ1t¨Y·?¡¯Û<Ω?ÛF{®æ\?¼‰R†'#?à\Ï(O?»·¹ïiH³?hÅM'¯ê?Rá«4ƒ`¹?Ài‹q?ž)-6I1/?ëá`—^?žº%Ý£%?x+ZƒÒ…?pvçƀàï?×g½Íwå?È´Ôn½ß?äl+¼
?ȼ-¥!.›?‡|ÝÅDLž?Nºàšÿ?Õaš&Ý:?Äáë¸k«?äñ"¼»?ÄØí—r¢à?¢ƒ¤sù?˜Uq«ÑÅÿ?ÝDù":ã?Á°/¤´¾?àW+‰Vç?ÁSØöŒõØ?DÌêU
½h?5ÈdõqÑ?ŶÙjìÞ?ªárŸzqE?êkқ?ªïßË|÷•OTHER4FGL J1845.8-0831?í"c)›ýÀH㞠jÀ9ƒºéuzÀ;RALÑiê@#ï{M~@©"˜€•?Á"©…JV?Öå-a4l@PÔ~qõç@û†°ð?ïöׂˆ[¿â±Âëc'¿Ýt^ÁVw¿åÞ¯îo´Ä¿êîU'ÙŒ¿ïú–ŸVOTHERspp1FGL J1846.0-0831SNR G025.1-02.3?Â4ˆN\s?¯®ð¸JÐ?ÈQvÊâ'Û?ºw}ˆQÀ?å^ k3Äl?¾#[[½¸T?Ø羙òô™?ƤË?¯@÷I«£?¢ÖVt'	i?ᚌ£'êú?ÅÜáøƒ		?ÓhúƒP?®]ùù^XÙ?Ëî96µý0?¯ãëoû?ޟèáˆú?²˜¯ ØWc?Ú	¤*ä|Ž?ª	bóGéV?»­Ê}Î?u¢øôæ?ßϨãþ?¬~=âR‰Ô?²äIi4à?¤E§Ç2BÃ?ʉ|öH‹?¾[Åxš›?çÒ&q?À"‹4H~k?ÁɞÉH!Ç?¶±U<%Þ?¶ͺ£û?°ÓøCAJ?èÌ~–3¿?»sKÀâwž?Äõác\ƪ?©Ûläåm?ÊXíP"±Â?°‰ñD¡&?ä,LS¡å?³Ýð£¦?Èl9[¼¹?§E®‹É@^?Âu½"Á4à?¤žž V?åG'C¢Ó:?²šË>"ÒOTHER4FGL J1846.9-0227?ØLÎ/d¿½
ò[ýËÀ8ï͂Õ2À9¥rE—¹Æ@BAê04ü@R+Ù¢ž%?ÁƑIhÿž?Ó'mb*W@Á"tŸ@ŠÒÒË?¬ÄÉ¿Òu`Õ,î¿Ú-³Âd¾ñ¿èëð«Ï¿ëîÈáÉ¿ëW€OE¸qOTHERunk1FGL J1846.8-0233cTXS 1844-025?†©I«hЮ?‰gÃQ± ?³"á'íÞ?Ãe¦1o·?í4Úÿ?ÃlØ]0?¥ñá,'?¨¡ðMÿN?Ã×®Ÿ‡'§?´3Txn?é«ڈª½?¶ð»=&~?²hÒRºæZ?¡¸âþö?ÏÊJ€F?®Î·ÁIwG?åð?>s?±Mjà×B?€VÑpê?cí¡*ŸøA?´ÆS ?"Û4Ѐ_?í''L ?"òð/Ïçº?w;7ü()Ÿ?tÉTˆ?ºi¸üòj§?½Ò(äA!?ì"RpÌW?¾-"¸´<?'2É<~É?—k	Z¿
º?ÄÀ£mFÄ#?»Pî£ô\?êFF~r)q?»Úûí)l>?¦Ë~ç8IM?"âԖ²Ãé?ÑG	ƒƒÐ?´qÈ™»?åï¼Øwó?´¨Ó/뿧?_òþ³?NG¯ì`kì?ºuñ™j[? åȚƒ¼r?졳ä
K?¡w¢rOTHER4FGL J1848.6-0202c?éø(¨E€¿ÔQlĤ_EÀ8RW˜mI¯À9¤mvûßà@ôüî@ç¶ãV|?Êk¿m"¬?ל;À•G@TUêî @z˜v. ¿íœ"N‰{?ï-ÇW嚿Ú<ßï¿@¿êh{œ"÷¿é5BEî¿ïÿ*±0OTHERunkNVSS J184840-020408<?†>I®ùó?'{Ȑa"l?'â»ëè(?(ŠLo{U?ï[{éQà?œ©}žXž'?¶´·ëqÜ?¹ƒ8®°·?Æù썘?¼Â®ü,`Ü?ç¤j‡Õ™G?À¥p`ÿãê?´È|f?¢âŽ¿›ÂÜ?À'Ôª".?§Qqž¿"‰?éW±Ôgº"?­7™><í?'¥Ãê<t?z»ù®=Ô?²éªÔbò?–€!$CÕ?휠p^ž?šTÏRG§]?wVI_Zޒ?€VJxÂß?'8"…³|§?˜îú˜8п?ïGŽÐÎö.?r³lL±?žªDñþ]ß?¡÷æö¬Š±?Í!RFZ¬?ÃjÜ7#ã?çÂYFËÉö?ÂwxvM(?¯‰ˆ®©ö?fšmóÜ-?À°÷örÛ?¦dm~­?éÛ)®?«?,}ÙÂ?vCHaê?g	V.'?µåÍæoŽ˜?£$ˆmNò?íÀ´‰ñ?£ÂJÿú©OTHER4FGL J1848.7-0129?ïÅP«'é￸}P·
HÀ8'ØÚø	À:S‰X@úFô±e@ND¬{?½©O€W–?á1Ú£O%@"]Ç5ï¦?ûøýlÒ¼%¿Þ›C<뙿ÛwŒ>] ¿ÓQGpĎ¿âgšþôgF¿ïü¸Lã¢?æ®&ïXOTHERglc0FGL J1848.6-0138GLIMPSE C01?|¿Aÿï?!µŠÐy?êªI"Äâ.?Æ;4Î,¸	?Äpágl({?Æ
™Æ?œoPC/Ó?¦^¼"§_?ämÎÜ`Wr?Å¡ñ/VÒ?Õ]mCzS-?ÄâÕßL?± õ>ÂÐ?ŸÂŠ/—'ñ?å!é8,0#?³VßÑ/Š?Ñsð?÷…?²1'ˆÔ˜?uŒ³ØÐ?aVÎWŒ9ý?к̾£Øü?²¢_4Â\?çxx‡P@à?²Á†Y·0¢?vìÅp¤D?Ž
¼1¯&?롋íxWÄ?ºõtò×^²?ÀÂjzæó?ºŒ´³XÁ?'×g/çÑ?‹Ôtdô?æúÑ9et?ɽ¶Œ÷þ1?ÓGO$UtÒ?ɗèz¹jÖ?£'™V9?™¤Wø4e«?æûÍ£-äa?´¸óWú2¤?Ï,¥òà:?³§˜G÷?Quµ\,?AºÏ9Ìq?ӄÈ|0':?¼¶í€?æ4àçƒSÔ?¼¾4\í°ŒMIXED4FGL J1849.4-0056?ìڊLl¹?'|[p>+ŠÀ7€3)'°À9¥€(¯K³@£‰™o@-"œ)–Ò?® è?Â&ÕøÎ]@—»s5@|s³Öܛ?ђ'ýîØ»?ì›Âhż¿àKH¾4Ù|¿ä'É oâ¿ç~þþx@ƒ¿êKý>¯"+OTHERsnr3FGL J1849.4-00573C 391?8œ²Ï?™1'ª?˜3Mꁄ?ª­nzÁn?î½ÓË¢2ù?¬ý0vM5Ô?­®³¨«³·?®ü€q9,?Ӕ"JÇhN?ÂXê>'z?ä[ Ò.?ÂӎªI·{?±8êç›Ù?¡[žx…à›?ºÑӔ3¡?¥²e
8^?Ꝿ§ùŒQ?¬iÒ¬Š·ÿ?˜ŽÊ±à$}?Á‡pãr?½°ŒØɎ?œe½±íF—?ë‹S™ßj? ÒóæîÁQ?'BJ#ûâÙ?æÖâÉe?ªÜÝA2Q?´&ªº>°?íÀڈC¨?µùƒ›ŠÈa?•eQm¤Öá?šÂ\êkã?׍û›—Jµ?ɳß34hp?ã×¦fþß?ÉÓ¿°.±n?©ÞI[o§?›~þ'(C?¹òQ5
?§
‡÷'?ë#× XÓ?«Úêxw?ýe>pŏ?pÎÕàL©w?Ã4E»å¸›?¬/Z/¨7?êêøûî'3?­[߸'€OTHER4FGL J1850.3-0031?ã»®¿rä{_ßÉÀ8Ú¬è*÷À:A
±3ê@¤WZn@g8¥Ì®?ÈÔÌ`it?ßÅi`ì©â@'ã'÷Ó@'Ź2;<¿çHGä¿áx{Â=ä¿Ûí$S†¿é_þ"/T׿ü¾, ¿ïõEâb`GOTHERspp3FGL J1850.5-0024SNR G032.4+00.1?z¸¸BÒ¨?xՙ‰…M¨?Ä[îaá¶-?Նou®­Ó?곒öߒD?Õ^µ3[?²Üëm•½i?³Lޗœáš?À+UR[±E?²"å‹Æ®a?降=ÑØá?¹këóÜð¬?°<ØÍô"?›%—´ÕÓ?¼®¤eç?¤A²Ûg¢Ú?êbY%c?¨'"ÆåÆÞ?¡Þ
ʕ{W?†n—'oN?³¸>7ð'?˜"c<ñû?ìk\Ïè? f²ºÈ€?vØw«·Z?mäòO±ë?³ÑKqyˆ?ÆX=Í?íX%£}ž?Åþ~ÖIÎ*?›@â¯s[Ó?œxº!ã'?ÂjÃ7¢®–?¼¦ô(¹æ?ê‹H›¹|?¼ûs¤ù…N?¨¹ÚY?é
ž/x?¼³rs?¦¹ÚAT‰?êèîƒÅŒ?¨l¹q
Nì?…9ÿìd
Ï?syô×蒱?µé\±çE?¢Å¶uJïb?ìíìiöì?¤)ŽQ#OTHER4FGL J1851.8-0007c?¼ÿÝRMw$¿Ã·—†nïwÀ8yN»NöÀ9ß:~_@UE®
@¥¦½n‹?Ð?'}rq?ƛi÷?'@hýAߞa?ø´ý먰
?ìûi,êCÖ¿çÈâ\¿ãÑ.~§¿ë5*Ø>¿éSÕj*@¿ïÍ;]ÎOTHERsppSNR G032.8-00.1<?¬Kux–Ùe?©]ËP4›Ÿ?‰Ø×+§Kÿ? ñƒ[+Ú*?íÓåKãr?¯R0´´ÅH?²{eÿrÃ??µ"5ô~y?ªˆ9Sè?¤âaèàü?쯆§
?·÷Êxþ??¼a`­"Î.?¨qo1zÇ(?ºb€Âv÷G?¦¬<Töw?é'ƒÑþ‡Q?°³šøn…'?˜/ñ,DX?‹ò¼žu?¢å&U—F?"®XHß?î' è>)?ðÄ£³xé?úèòzäÖ?ŠƒæçÄ?x˜9ôï?u§'?ïF÷}Ðe^?q°IóäË?ŸWÍ6ù/? ôâê–Bi?®:1#Â?± -ä@'?í!ŸÕrã¢?³«fðîÍÐ?¸¤ùKR[9?£1[éM?»Ÿ¾Tlœi?§MsO}ͨ?éwiÃhÜ?®éXè‡:?}6Ò«Ý3º?j«d¶M°h?¢;Xtúí‹?:ª åÚ?î¡ÜÓCù?î&,åOTHER4FGL J1852.4+0037e¿âz+ÙçVU?²¾vrÍýÏÀ7*'U¯^þÀ9n@V1dý@Ë£Œ·ˆî@XçW'Ž
?³uÃ?t#?Ƕ›Ø'@¹DŽO¹@&;Á!Gù?ïƒ9L¿ÚFÿøš¿á>f7l}Ø¿éâŽÕñ9¿ç֔–ûY¨¿ì‡{‰äðOTHERspp2FGL J1852.7+0047cKes 79?Ücõq&v?ˆluZ[Qq?w€ѹï?vºæÓ]/?ïJàb(?ÀÊþK?¦f
¸ûª?¨Ž¢ôÐæ§?Å4Ì´èÄ>?¸UC=dt?éLl'¡?»‹Vq_i?½¥¶â™‹?§ çe±3	?ÀÌG–Ây¸?©ÐŠŽ½1I?è7=ü1a?± `"΍Ì?"CG'
»?€nX,¤¿?¦æq:_4^?»Æ.ù;?í÷~¯»ør?•¼ƒ¥ý°8?ˆëëÊQ·?€Ò(ª6Öq?ˆïf¢äÆ?ˆä¥	#0?ï8'·8w&?'¥Ì¸ð<?–ÌSD''?šálŒ³;³?Áû0ÿ7"R?º4[/VT?êÊÑ&¦_?ºÓ6•µ«À?·lq]qgz?¤mc7?ÂPE©â×?«ñ"gjÀ?è~`"P•«?±=H»f»#?zû•N闓?nżÀƦ?¬#wUÁÍ?›ú«m±¨<?îÑcƊ$?Ÿ
ǕŠ©,OTHER4FGL J1855.1-2243?î¦i¤g¦À%цÛPôÀ:f	{¸À<C{cM­2@p¾†¸ìE@Èêí+?ÅGmgaŽ?ÙÆüÿ¦@ ü ÏîÀ?èÍ®z§?ïÑGP ©Ä¿Ü´'drñ9¿ÜÊ1ç٘¿àÿà?Æ>"¿ìAÿ~Ñ¿ïÝv¾"eOTHERglc3FGL J1855.1-2243NGC 6717?ÙWÿ'¤?ÉȬš ?Úo¯˜çö|?Éf6sb+?Èp¡ÈèË?»4!¸À?Ëâ*à†ñ?Ç3ë°ÎЙ?Ø}‹®@çô?ˌÚ,.?Úƒ<Nԓ?ɏŸôì?s?ÚW|qHJ?´QéöŒ
{?ØVò*)t?´kO	rÅ?˼£"Ƀ?¬Pú}
÷é?ÑUÞö½Xˆ?¢ÆõfVÈ¥?ßoØÁ?§ý7®ÛÎ?Ï)cEn? ü/ÅMN(?ÏhKÿîôP?Ó;º?ß&Œ7A›è?ɛþݯâË?Ñ%MÈÆéð?Áˆ(Ë?¶€°kº…š?¿XP2.?ß´€Ê.¦ ?Λøâ‡ý˜?Ú«SYGš?Ìü'­ßC>?йNë w"?µUÊbQhY?ߚù|>{!?½"c&•ëå?ÏWo0Bµ?²YÏ>T"?¹Óß{%:L?–¶˜÷ÀèÔ?ã>H»Î?±*Ô	Å
?Óf‹À§Ð?®z‡v$¡MIXED4FGL J1855.9+0121e¿ïÚg·k³û¿ØÕ[½•øÀ5pfB
gÀ8¡%µ¿j@	-%R@ê쑎2?™=#¡ð«#?ÎÝöjÕâ@8oÏå†6@
Çf,"ÃI?ïÀ°^×ü¬¿¨šÜ æ{0¿ã^ FÇe¿å׈b9°ü¿ëS€™¿êP="OTHERSNR3FGL J1855.9+0121eW 44?žš=SS¬S?©ó4«wª?éÝþÈiÞ
?Ëʎ2wp?Ä´½4\Ã?É*fƒË.Æ?wWýA]Ñ?Ž;®˜3†ù?ë%¨ñf	?¿Žw—uŸ?®ŸùbµŠ?¿K`ÐzV?¹ÇÜÉ«@q?©{ Ø@i?ßô",±-?·Ö"Kµ¨F?ٙ" ä¶?·ý–,³×>äËØÖ?ß>â»I2
…?â«ä·Ë?ÀÄÞ!;?Ú¨ãW¬?ÀÄιêz?˜4N€‹ð?ž>ït¯ŽÕ?êÑýÔȨ?đ,Ö«P"?Á±~ßüKã?Âð8)ðœé?z¡<ƒ'?¤ÍvT•åw?ì"ÀN‡?ÀkTø)òÃ?½ª±faUR?¾Í…øZ¢Á?³®ù¸W?©@Eø)>_?⑨Â胞?½x¬Øc?Õðð4¨J¯?»{^ä£>¶8@Cæàx>¾[Ø?ûm?âšÌ}­»÷?ÃÒ£éFÖ?ÚÊaw.È?ÃÒ¢`PSR4FGL J1856.2+0749¿íª¯ˆ9Ê@ö>e–\ÎÀ8v(]íÀ:3ùÄ|œ3@&#«UÚ@(îñºÂß?Ù¥"Ò?Ò^zښ@{ؾr–ö@á
s(?â¿âT'nâlq¿ê3âààU¿å8Yã¡$¨¿îa¡Û‡{¿ïÿCÂw‰NOTHERunk3FGL J1855.6+0753NVSS J185612+075340?µ¡¸uG˜?²4Âæ€8?Ò¨ÁN5å?Ê(3žñ?ä}hB[?ÉÑ.Ñy¯Ä?ÊãõEÅd¬?á–W¿?Ô1	?Äöwºxø?Þ\è̐D?Āhtwe?Ë'æÐÌ?®.`î/ݎ?Í.ž4D;?¯Àîl5±ˆ?áê^íî|í?³"ý&ó?©èò]°(_?‰íšãö©?ÄÖ¢:ÊM¹?Ÿm*ÆÇ?é+ÈK;pL?¡›äh?¥õIá©{? £l¨¶P?Ùm9æ3?Í­ý I?âtՃÄ_?Í/†j…t?­9ø`ƒ¶I?±#'CÅ/R?ÚT
g‹nL?ËÑüÀ
)g?áYÆÒ%?ÊâSoœM²?Â-N¼?z®?§– Eù<?Ðހô‡%ú?³–*iÚ?ãkÖ¬ŽX?µṆ͐?‡µg€lÌÝ?p[E0ð½Š?Ìe¡`s™f?¬6õšØP<?è‡Â	áfs?¬q'¢+#õOTHER4FGL J1857.6+0212¿àü¡ž¿ØÛaåùÀ7••žÀ9oAÿ~ÐÀ@p7ÿÛ=@7ïZ–O?¸#¾5y?Ö½"થ0@ ¼cñA \?úv8kX?ïʙ쥰¿ß4È<V¿âùÁÍjW¿éöå¿âÙ¿ïÌn"rp¶¿ïЌ­OTHERspp2FGL J1857.6+0211SNR G035.6-00.4?"©8¦˜8?™ÿUoíJ?Þãx•'ú?ÎÊñS´?ßóQóàƒ?Ï
5h~?Œ—íÞD[?Ÿ‡7K®š¬?âõƂIµš?ÃÿIâ!GÎ?Ù/³Œ^ó€?ÃꠁYÆ?¨üœ»n?óeñà?â^'!« ?·f-˜úÁ?Ø@EJ7Ñ?¶cž ó§?IæcÈ(Y?4Ã2öÓ]t?ˇ:$?§´gڒ"¾?é8B…Fây?§ÂYÆÒ%?Ž‰¸P×?·j^×Fm?à1Ýwڕ?Ë`‰f$ï?Þ§÷NðAá?ˋ_[҆?x(ºj3?ƒµ˜ûÔj-?åbÀJnŸV?È°x€?ÔÙ܃Ùw?Èã†+—?œ¢æB–\á?"'B¬#¿?ã&ù,boÈ?»¼}ýº^?×çßC-7'?º¼s‰öŸ•?#›ËÂ?N.C¨?Ñtb£
`¼?µ2Yb¤?çD"ô» ¢?µñ—ëMIXED4FGL J1857.7+0246e¿h¸.B#49¿Âÿƒ
6À7ô'|À9¡v¯‰Æ@ ê¿É.1Â@ü,9
ä?§!\=ú×?h'"èl?È2<Tì?ý‹ÐÓŠT¿ïàsÞ-è?ïÿàU?Íu¿æ=^ä'å¿å'$óÅ¿à™[á}3¿×²í'¶'OTHERPWNHESS J1857+026?yˆ…±ôD?'|
[Ïí?^=§xzö ?~o0'Ù†Ñ?ï½Ð)<~$?Š½¥ÇRÏ?·‡´¿ºÁ?ºPí¥_‡?§"öÜ:´ú?¨CsŸ€ž?릛–žè?¾ž^X©?³€ÇT²Í?¢Ýb}?³ë×ìú?¦IüûÎ?ël#"·?­d"4lþ?¸‡29q?£'¹ÅT|?£EP›g¾Å?ŽPEÒB
´?ëºÄ´Fæf?§æÜԒû?
<£öõ?£VÎ铟?gˆ‡`À"?w)t?ïtCd6hû?¤	OÅCß?²ËÿÈLµ?³M•À¡9Y?ª(e‹h[?³ Þwén?ì '›X?»u…›¾j'?µÛ;\ÜÖ®?¤SÂíøVî?´%bR­m?¨ztcŸÐ?ê¿ìIóF½?®ˆ«"€?©ö¾zC?šI&ö ?¨ªÈf†~?™{Í/?ìÕôç%$?¦=Cw6óOTHER4FGL J1858.3+0209¿ÞˆSÇ@5¿áu"@òŽ}À8øéëÀ9ûïº7žÓ@!ÅÈC¦@¤ßÎ1PÛ?Ùc²ó?­çÄgB?äÏñå‹	´?û3r@9V
¿ï™L'9«?ë|vÕIs?íœ&¨«¿á1J$ç@¿æóé;˜\ƒ¿ïú 9påOTHERsppSNR G035.6-00.4?‡øw–&¬ï?wc[íÉ?b'6o¼?xs³8§ý?ïöë%Ê·?†%ƒHÿ‹?´+"·+?ºxžÙ?˜+"@«' ?žÕ? Í?ì¹Aí,¶?¼û=^Áh?ÃKÅ÷×£§?ªx˜úڞ"?º©¸œOg­?©ÇBçP;?ç××o	š€?°çK)7?¥w™-m^?"eñ•f֏?'f̚OZ‡?x3ÐÁê~?î^ôC֐è?—fêg3ã)?‰N"™"Ó?ƒ¦F§äs?zRÜSM?­õW¨?ïf ÒÇI?®"LÊ%?²˜˜I¯ÃÊ?¶¬Á"®!?›^%ëˆ5?­ZD4"l?ìÑøíUó?º7Ð*>0×?¿àΈ
?¥¸]Ðs=?º²ØHÅ°h?©a,]ߌÌ?譋%ãiq?°_æÌP›¼?–æk\Ú?ïÊð؈?zÒ´àÍUÎ?}2öMß¼?ï"_?D}?'ô¬Ö0z|OTHER4FGL J1900.8+0118¿ê#O»T)x¿÷ìqþJÀ9'J HÀ:HgÒw0¹@òÉÞ/ö"@f?šIÂÂ?Ñ£#=­?Üû=£z@Ͼ¹ä'¼?þïSZ'É¿¡…¡êöÙf¿«ŒÂƎš¿ä¦ˆ*¿ìÁÓ_
+¸¿ìšƒ¿<ÁQ¿ïğá§OOTHERunkNVSS J190146+011301?›õ‡Ó‰Ú~?•S³<u)·?–ó\iɃ}?•3îÓçÐ?îh¸Ýùè0? íC|æâK?Ê~¢r[<<?ÃûwUÞ.?·WÎ)£z_?±ù­z?æu]ž'5?ÂbçX
Ð`?ÃÝ#U´VM?«K¾6µ]j?·ú;l7?¢5	ÌHâ?è	o¼•5ö?¯$mÍ?žæm‡&?—a¥â?µõ*Æ\ƒ)?"Þ"W#?ìJ'>eôÚ?–nœM¥£?‡pŽø?‡:½??;ÍÌ×'§? RÞ×ã?î¹µDF2?£"_ÛFˆ?¬e–7ì)?¬fUÚMn?»H°ÀI(?¶¾ˆ†Û×?ê؝$C	?¸Z¿aï?µxÙ@äÒ?œ¸ìÀêÊ?¸99Ph?¢þ)¤Îî?êNå"Ùô©?ª)²OÖm?~¬ì…ð\ƒ?f'fU9ºV?·÷R䔼?›zz.?9™?ìûÊ#­¸?œ2¹Á%{OTHER4FGL J1902.8+1451¿î.ï¯ÙT£@	&A³)À:l*pìÒÀ;½—Õt;@ cȑª@Œ$ÞܙÉ?ÇÕ{]2?[Ä}Y-T?ª!Þ:ø@|šCã…?îb÷ç,Êc¿ê»ëýê|¿ÜÔ	­þ«¿à@ï´XaÁ¿à'ààUÚ¿çt¨+,ÔOTHERunk1RXS J190249.1+145133?éƒ.•Œ?½K.ýn€;?mÞIñ>‡×?aêC4òøÉ?Ë2zì!?½.ê}{šš?åþ»Æbâ?Äò²šF'¶?¸SÃ÷f(?'[UV±?ÓÆEʬ?ÃõXuü >?éQ^†Àpj?­ÖÃ"üp?f(¡A«?…¯³ð'7?ÈÄ%"=0|?­|^÷çj£?êD¡Î­ˆË?˜#Óñc—ð?yÞ0¦~Âó?ZçSÏ˅Ö?ƇAIû?—Îòæ¶E?åq`;‡ž?õ)J¯¯?|Ó¬â
‰?y%šI'÷=?Ôªx‹ÏMþ?ÂéGÌ?ÝÉol—?ÅtÉfÌùÔ?'D•^¶¯?¸d6u›?àìWpn÷?ÄâOmC?ã/Ûë¬>•?´B|Ë,'?›–•'ª»K?Œ{Œ•š°?×æÞÏaZA?´:Èíˆô?â%«h׍?©<Ñ׎º?ŒyÐß'® ?vÂ3CáÆ?Ûæ"£ï?©
Çc¸SMIXED4FGL J1903.8+0531?v'Ùèemç¿ÏPŒŠgwˆÀ8P*|«LJÀ:ešŽŒ@ØéH-–;@Ù7fžšŠ?Àä8yC7ã?ËQäç ¹@ã\[J©@˜/…)?ïkV/Ž?×!¦BõH¿çÄM¢J¿ç5†_*2¿èa.ÿÿe¿ê¹'Ñ!EOTHERsppSNR G039.2-00.3?º©ž÷…?±H€YNe?¸!	"Ëò«?³HõÕ><O?馫U[?»Ò§Ül@à?²––p@ñ?°Ûõ9^­?¼gÐ|bYÅ?¯HjN"»þ?ê E}7¹*?¶|vDÁ*K?·¤YŒÊdy?£—ƺ÷Ó°?Á²—Æ?©ïËKå©	?èžô(u-î?¯–Ç¡!ŸÎ?£T'{¯Ò?"–ø´=Q?¹Ä¬'Tƒ?'t½å ¦?ë'!GÎJÑ?–å,Šº"?ªÓӜÌÇ?žGWUÇõ²?ÁƒWk^?¹äe3¥7Ì?ê¡ð;x?¼š9'ø‰?±*¿M1?¡ìßÇ
`µ?½Nme"?´Ó/<ñ‡s?ës¨ï¢æ?µÓÓ¸_" ?²n}ÝIžd?ž Ü´PÓ?Ådçbq±–?­ƒ;T‹?èXök¬¡^?°æ"ü"?…Ü/Âð'ë?pUÿ{ù³#?Àh¾Q×/Ÿ? <aJÁÇ?ëŽ_¬bôí? –	ÀuROTHER4FGL J1906.2+0631¿íG¬uÐx¿ÓVŠüñ}À9½1NV¥À:JNÇä/À@%ž©xß»@˦"c§o?ÔSs¯ûî?å©Ë@Ó@;ŽK‡½Ï?þ‡ýÈI¿Æ(!\F'¿ë¾aÔU¿ØÈç$'Ú³¿í!Äuæ6¿ïÿø="ßE?ïÿ /ÄêOTHERsppSNR G040.5-00.5?ÅÔVՊòž?Á4…
ôÙ9?È7L2º	?ÈUªñª?ä}>TÖ?ÌÓó8¥l?Ä/ÒŽC?Ãû·µ¨1Ò?³;N
=Ðý?°>§zí?茥Y¸¥p?č×?Îámz¤-i?±.g·^#?Ä~xôæúÔ?ªøc	¬Õu?ã(d5ñ?³n‡§t?¥w‰û2Ä?'?楲?²yîE"?—xP[¨–c?ìf8"}¥À?¡9«Ç—Ï?³ŒõÞv?´K¢Î7÷?Ê÷q³møx?ÉY܁íø¹?æÑñô=mã?Í*F/dF§?¬-ÒÆíØ?³ÚZve"?·'•<öR?¶•¹J-"?ëL*zýÍ ?»ßú¸(·?ÃnжCüã?¨ö?æ3 ø?ÆÛ[P2ÈT?°´°ðO?åmtþbN²?´š×g›ñ?€:²9=ÛM?oÊÇgÙ?´^SÈT?¡}Îꌺß?í>‰li¤x?¢GäÔçŠOTHER4FGL J1907.6+0703¿ïC
Ô²|ó¿ÖÑ#^))À8Õi´Ï€À:ÿ¼ä!}@!L/å¾@—ºÇç‹?÷ØÎbÏ1?»LemaØ?øæbÕ¸-Ù@<‰Ên£¢¿ïÿÆ¿l'ú?ïÿþR€ÖT¿ê¢ç@k€¿æ¶a@aÄì¿é0Ձ¥‡¿ß7Cõ"VOTHERsnr3C 397? ×÷2²÷è?©V.-6…R?¨ï	»$4¼?¾*tXþ…?ícñ>
?Á&_Ã
#?²‡í|9D?½*ˆ>ÓOs?¨Oe–MWù?²[PH¯Ö¤?ì*÷Q}?À:[N7ùõ?ÃuV¦!^Â?ª¼T3ÒÎ?ö¯ÆÌ?­í§›ŒyP?æ]üªµöœ?²ß`³b?´EðÀÇÜ?£B¢0Ôϟ?ïÜÊ°c?†Ÿ4š-Â?í8$WŒô?¤QàcÖ´Å?¡[ e•Ïî?­oȚ Ç?­VÅÔHÎ?¾Î:‹I?íٜF¥´?"VþXNå?«k.ÎÔ̼?²Š/vÀr?°+[­¸¥ò?·r§Ñ
Œ/?ìCá$¤¶?¼ê'ŸC@‹?¿¦ÇCdÈp?¦´pA•?ÅG·gä?±-ç?æ¹9W9¢¹?²õg@£V?¨tc؁1?¨°Û¢Ð}?ƒ9™MJ_?šÁF˅=Ü?î2Gk3?ª¸é¨/OTHER4FGL J1908.6+0915e?äñ(I²?ۆAãz8UÀ8='ùCM]À9ÿ_tڝp@ IË%,à@$Hdà?àë¤Éx"v?Ҁ3â/µz@¼`ˆÖÓ·?ýCƒÃ˜þ?ïÒ7y…¿ádƒ7W…"¿äLg¢%¯<¿æ¢_I¿é ÃÄæN?­[ƒIBŒOTHERsppSNR G042.8+00.6?¬ƒ‹+Àîµ?ª uR¹Ð?§4J±h9?«1Þ0Á"?ìĂ¢}±?³ïOõßá??­¼dvëý?³Ì¦k|4?µ
þç<•?²z¯m?난yÀ,Î?ºƒ½u}?¼ì¨<þÎ?¥ò/1Ø¢?ÇçtT ú³?°
çìˆ?æhãánù?²v…Ñbê?¢ßš+{3?ƒ±í9ˆ?¬@'X—½?—z<«-Êü?í
ýGz#C?šH~êƒÑb?¦w"Ù´Šã?©<vȜ,?ªb³/k?®ÍŽ?}¬D?ìíp?µÞ#9g–?"³zgæ?¢­Oß,°?¼¥|¯[«U?»´,9fJ"?ë0]:v?»þˆº+èð?³·†PK#?Ÿ(ŠTó˜?ÉqIƒ×u?´ãeQu?ç,¹î	¿?¶hf*D¢?"©-j¯;æ?r|]IM?¦ò³Û?¥=W¥2ð?îMLN‹?¥-|d3ïOTHER4FGL J1910.8+2856¿Ò	*\[1@!ͦÅÒÈÀ:_:Ôd¬À<H>¼(@!w×Å#`,?ú+RÿTÿ?ÅÛìdí•o?Áq¤ƒ³ÿ?û°^òԞR@©…—Ùûß?ïøøo"¿í¦÷P.½?ÏI5¾}ԗ¿Ôÿ©ƒq¿×kr¿»l¿Õ/â{ŠºÚOTHERunk3FGL J1910.8+2855NVSS J191052+285621?&ˆCË?¢¨%y/?T	F	­ˆy?L4v
øX:?§ÓcÏ?¢x6}­L?ëë"Û	?»ùáò'ž?hªW4¢Ò†?qþ­Ïˆø?¿Þ†nÕ±ß?º–›n?íÑbCœQ?^¥ÿë?er"ØEÊ?^íç8Í?°É_fIË?9RØ1]?îÜ{gX ?w>ì;qO?[D«Ô R'?@{C¦ž"í?¡^)v³õí?víÂg |?ë.ÚC¶kÀ?ºDŽÑG?mOfÃwW?hÃz'â-A?ÂÏYUBü?¹ïÔ¡Ç)?æŠÕߣœ°?È2''ÈÈd?rg‰X>‡?'1€•6""?Ò ¶¸öµ?ÇÝæDíð´?êOw
AuÛ?±T""?r!M«Ð?j_>j[Ú?Æ1_nòÉ?±@ªd‹þx?ìۗÔ%9S?"ÆÎí¸
?l8¬Néü??Z˜š)->0?¸A{ý'"?"‰IBïXAGN4FGL J1910.8-6001¿î‹JáЕÀ9¢È:£jÀ:UàñFÿ™À<¸6<Òï@/H—H†'?ÿÍÃ7!Õ=?Á¯þµÓ?àݰʹ@œb^™éK?÷Ø腏÷?ïôºâ"Š;?Û:`¤¬¿ÞI
DâG¿å¾å¹,ÜØ¿ð?ïŸJžê	OTHERglc3FGL J1910.7-6000NGC 6752?ɶÿÆ?ÄLüV–ÿO?ènc²¤N÷?Ç.äw–î?¢=Ȍœ5?£¸š­>¹?̒ÜL|Z?È.1Î{šø?åæM´T—?ÈØ	èrUï?·¨aÄb'?±Ã´+]L?Ê<j£{´p?¯é'Æ0Šé?ä™"àÈ?³«ó÷ÿ˜Œ?Ã_C
+Š?©V¹nLï?ØLh[çú?±\Ö´Þí¬?ß'lŠ0´Ã?³BmÍ°?ÁV3Ïv‡? ›J>.è?Å0¢—Ë?'wØÃiæ?é1GþœR±?ŸG¸.
?¨(örFº?§7a±Lž?» ÷`8Û?À™ÑÃ?é~Âþ—Ë?ÄÓlµF.Ÿ?¸Ó‰	K?´|±Ñ½°!?½ÞÅ÷à:­?¦ÅJÍÑÕ?ç¤J®êu?²ª?€µ?Ât¹T8Ö?«èJ¾«|?ÂK&ïØëi?¨kÒQ• ?å´ñÊï8?·ªå½Ñµ©?ɦFՖ9?°£?j'PSR4FGL J1911.0+0905?çÔ Û¹l¿ÆŠæ¸Ü*
À6¦»¡+^SÀ9©\¥"›@ \Y(eNä@þš9҉¥?œŽ÷Õ9Õ?¾f{µ*Ó@#,Ùb…U@Y–8¼?ä²Àü§†?ì@֟^'¿àó\îî_Å¿âYöKKWí¿æ•V©Zý¿ã\νgÔûOTHERsnr3FGL J1910.9+0906W 49B?†£¸–îê?Ž³{hØ?ªZy{ʄQ?µÐÃ#5?íÿɅ´N@?¶‹3²Ù‡?+}õ2Î]?—[kF5t?å¼Ydÿ?Å%áŽÙTÎ?Ӆ+ãތ=?ď'8?¬lÑõ·™ã?¡I±ëC17?¹üë½A®:?¨:}¶Vl?êù•hî'+?¯ÉœÉRX?pù٘]¿"?V¥ô?Ú7‡*×,?°`–M‰Ë›?âÂH·©Ïó?°e©Ó8ý?à²N8€?‹"I
j?±.Þ¡^Ր?´J4샼Ý?íZ¡c^ìl?¶	/3X?…Dsy(Ƚ?—S/%R7?å[šãú"?Ë:J|ƒ'Î?Ԟ¦œ"ÿ4?Êqx4¼l¥?¡'·ÙôÉ?œ<š]?².ȯ ?¤ˆeϪ¼?ì¨}¾'îC?ªYìˆémù?SњÔçT?C…˜[–¼E?ܤOS+?¶.q'Ÿ?á£ï‰mÛ?¶0|Æ£]«MIXED4FGL J1911.7+1014c?íèKgvJ¤?ʑb}ù€	À9"¤ÏWÁˆÀ:C_?*¸:@öÐÑê@ÖÐ& û?ÓéLçvÇ?ÛÊދ?@
¨d©ÍÄ@z|rí2?¹¨w­áz.¿ärÑCT§¿çò›Þ˜QE¿çè§ü2ì¿ïÿàè@?ïí—䱛OTHERunkNVSS J191157+1007208?Ïärxöê`?ÅØiIUñ?°"Ú¬¯,?²Có3?åôHã?ÇÕÅCìi?Р×!J¹ž?Æy±1eә?­Xµö1û?«®?æA_h?åÚ	Iú?Åû
6»?Ð}iÇÍg?°˜îĆf¾? ½
½?©³2KE'u?ãt[ت?³1+ô÷ú}?ºòŠÕBl?¢s­m?§eµ?ŽÛ2³M-?ë+SSË?j?¦¹'k#¥Ò?ŞÕ:&
þ?Á#Ûß0Éï?µ
	я´?¶PçÆ?ç÷	wUªŠ?Ş~v—P?»
û§fòä?Àqz^Él¤?³ÆéÇ¥Æ?¸ÕŸ(j8?ê%cQç†ë?ÃÞIy1þ?Ã(97·°?§£\dO¢å?ÃbuJ×?«¼gÚÒÎ?æb°TN¿^?²ü›xj?§?šaQÞ××¼?‰¯<Çp<_?©%hRü[™?˜t8°!z·?횞ì¶Ø?žËF4αOTHER4FGL J1914.5+1107c?º¸×âÕwÁ?r;éàåЭÀ8þ~Ä+=›À:mܺ€™î@Ú¹w/Œ`@¯P]¥?Ëô²YƒÿÔ?ØN»{ì‹@D7£~ö?úi#͏•_?ï¢á ÁÁ¿ëtŸ¢G¿âñ—‡p¢¿å߂ç¦lç¿ïêX~FVü¿ïu üÏÊOTHERunkIRAS 19117+1107%?«çèEÉïÀ?¬ÑO³.†Ÿ?²gd¿z»?²Çj¹yŒH?ëô"ø}³=?ºÃ¦s¡Û?³õÒ$å?²ÆCÍ‹®?À«Êö«9÷?³ÛlBç?éV[Gé–?¶¹ë±"ëä?éšûeÞÎ?ªš©ÉnqÃ?ŵÿËý™ô?­Sq‡¥Ó?å¨N'!Ï?³^³ô^˜.?˜Ü?-'Ü?xÈ+çˆ9ž?Âm9SÞ¤f?ŸVêo
~þ?ê¤JÉ8(ø? Æé/šQ™?ŸŸÏŒÇX'?œ=}ùzá»?²´"ÿ
t"?®è¹YPø?ì¬nã¸v©?³2F'-uÂ?™¾Xо®?žžå·>?Àªew[´º?·ª¡ö"¯@?ër—™†œ?·ˆvL0²?µùöðoÈ?-)²?¨™?Å°D˜'º§?°}·æ¶­Ò?çÔ¯ûìÜ?²?Äæ?w5U
Õy?`®(PvŽ?Äȍ¢ëR?¥sÃMöl©?êÊc2vÂ!?¥¦ï•ëwOTHER4FGL J1916.3+1108¿½Y ´"Æ=¿×ã	
¦¢À8hjª˜Å^À:#ˆY@û®a§»@$,<žìÀ?Â}BJþ+?Ï©ãhőD@€aº/;@£ -²k¿æprÄBº?ïÎ<~`ƒ#¿äyh6J>è¿ê×0h}—Û¿ì/#¿!é_¿æ=\aª¿ÝOTHERspp3FGL J1915.9+1112SNR G045.7-00.4?¥²–ˆN? +)¡Õvk?±†Àî°ú?¬z<d¤â?ìtbЌ?±h÷ÒÔk?´"ŽfÑ?±\[ƒÈò¯?ÇÄÆ+?ºv2P#?çµL,•?¼#±µð?½O¤SÃâ?¦©'þ"næ?ÆT¹þòlw?­?'I³?æÀÜõË?²)G‡Í&?¨p`eE?‰ÊŽ€ ´?¿ÕìõÐëÚ?—à·šít?ê|K["F\?×¹¡2`?'0ñ^ñ­?…Ò(jþÉ?¸iØû¬?²GòO®¸?ìiW½0Í?³Y(Xÿ?ÈBŠ]?œ!;ÝþWÇ?ÉÒ~I~p–?À
æè¬Ò1?è¢r+t*¨?¿¢ÉMÄâ?²/yJÒà?›Ä¬ý*‹å?Çy#\Ð?¯¿LÀÍæ?çÛȐÖ@?±
—M|2?¾Xi_'?u$uï‹ã?ÂƃÿËÊ?¤ŠÙª"7?ê×ež"(Þ?¤ÓºWÎIÚOTHER4FGL J1917.0+2245?ì0g>'­ï@v®b~zYÀ:Rß&k¤"À;›%d=—:@îƉ;Ók@"%kÊSv?ƇE¯Ç?Š²?‹cÔn?Í©Ä_Z@ÁÛÍEÄ?ïÇSó¿ãt;Áw.5¿ì¶À5¯å¿ØýŸ˜¿ák¬N"r¿ïÿï0l¯OTHERunk1RXS J191710.2+224852?ݾ¶Eï?Åy^!Áè?mt@(ïú?ecš­`ï?áS0 ÿ?ŅŠõM/Å?éèàyÛkÕ?»æ Š'û`?y¨"Jªw?¶¸t¿/?Ǐ9tÑõ<?ºÖÏfý\"?è2Ñtãh?±'.ÍÈË5?'þ…_-•˜?ˆä4,oÜ?Ì×è
3Þî?°‹÷-â?í¡yZgˆ-?ŒM5Þ'?n ,YV?Qz'5SÌ>?²)s:?‹ùS1üE?ÓKÀ"‡b?Ä÷G愿ÿ?9Â¥sÅß?|	ã㲌?æ8«`?Å*֏»–¼?ワ³ ?Æ{˜Çâ'A?'!"þ-?ŽÍ·¤ÂÎ?Øh¶h?Å׬øy¬r?àÜÁó'ü?·¥à®¦Ó?¥A›÷Yø¡?˜<4=¿ì?۞H™»—4?¶y!	ë´?é'÷AÃ^?¥Ï'‹äd?‡¡Ù»
¤?s±.YÜIª?Éæg~ûo?¥w% VÿÅMIXED4FGL J1918.0+0331?Ãö
uq=§À-ÕM¤ÎÀ:Tâó¾ýÀ<jì$·@"*ÂsW‹?øé¥e¶š?Ècêá	ðš?Èî ÝÓN@B='1Æ@Ýw"áú?ïÄ:Âs­w¿ë
Шú_­¿Çè´ÊL"Ù¿Émêi?à¿Ò€XÀ`'Í¿Ü'kÏOOTHERunkNVSS J191803+033032?ì½RZãè?°PÆE"?fhW#ʬÙ?Wé}B…'?¹b*mÙûž?¯×ÊÅ -"?è¤r]?À׳LJ?nÞ$,þF?v ‰Ó ø?Ï
ˆÜª\Ø?À§Íu$€y?ìš9›Æß<?£¥¸ì8?r㣠¨'?jK:ë«5¬?¹ÿøç:"Ú?¢ÔãéRÈ?ìϖ§]Ý?'¸Vëk•È?jPÌv'ºÌ?Qõ¥M÷Ò?¸°ÄaüñÄ?'¤À¨<?çv6¬Ô#?Âp<NËü)?wº´å-?lüðÚ´É ?Ñd+€-Ú%?ÂG"ºêD?à®Vü!_?ÇrÛ'6-l?p²÷Í @¨?Ap/4mg?Þ¹×rÿ7>?ÇTñá{§ä?ç¸\ÀuP?±5ïWêŒK?'"z†­{r?yfÞ"2£?ÏöEV¡Lk?±!–ûL?çgÞ·
¦d?©ó1ZRøD?|ƒ}C1ä?mî8ïî	'?о6wòf ?©ê,TØۊAGN4FGL J1918.1+1215c¿îúd×ðí¿Ð?ºà¼ôÀ8½3€`°À:HKjaž@!"å]<@¶"}æO?ÊJ¯;At"?ÝЌÀ\¾@±JÓbé@ ,|_Ìï¿àÓí½Þ€¿âzüö`D¿ä'§èM‡¿ílzFíû¿ïúÍ%¸ m?ïGnß0҆OTHERsppSNR G046.8-00.3-? àtfÁŽ?¡Þ@Œ?¼µ(fâ?'kõÀ®'?î«›Uä?£UfNh˜Æ?ÃÎXI?〿aî?¾‹ÿÆ&óè?¶+×ZîƒÄ?ç:éÿsÏA?ÅTÍWT?ØÎ:¦?ª.ÆG9´Þ?Ãaî½7ƒz?«Â¨"±×?æ6Þ­?²5Rs‡–?¨kÑþB™5?sJwùh?¶C,:ˆ¡?™ò­®Ð?ë°ÝX"È}?¡[œvë?"K ù–x?"«mƝÚ?Šà¿Åh¯‹?9À_
ÿ?ïD7Ôqu¨?•V—!«\¡?¨ßj›?¼"?±-ÀÃ×T?Á{(?d?¼äv·—[|?ê,¥÷²Õ?ÀªyÚa‹?ºi§yFø?£ז½6Ñ?ĦÆü†×S?¯…°Ýǵ¦?ç‰Q4Ðí?²ÆBÉ°?"_ؽyÓ@?s&×ÁX¶Œ?¸ló_%?£ÌpÌêւ?ì â1I4c?¤®~Xû¸OTHER4FGL J1920.8+0418¿èzžk²ÍêÀ>ˆXÿu—À9¨" [TºÀ;"×I''?@wì…#ëÃ@]ô!¥l6?ÍM›ê+ØK?ѳ]û]ÙÐ@7ã#Pg!?ý·ö|b?î€m®YD??ÛobäPÌ÷¿ÛÏ|'l+¿ãÿÜđ•¿ë	FОé¿ïÿ n4'OTHERunkTXS 1918+042?Ñ{RΦc#?·ª°ãÐ.?_·6ÓË?'yðt^É?æWXÞàÂð?·Ó›½ÉU?Ô£c"3Š,?À9¼¢Á·?² ú¶êã8?¦ x¡uˆ?ãj.߈ރ?ÀQaý &¼?މwŸÁd?²@Œ9ÿ ?¸Xé\¯Á?? ¶öo0?Û`N÷um?²$™våãÀ?Ù²†¼z?¤±‹úZà²?Á°
"óS?™0؟oÅ«?ÝuschÉÝ?§Ê­XŽ?·v¯—"Vì?¦ÂÒæÖß?¤s7†X³?›øÐ>œ?ëÉö"Øzç?®Z,fä?¿"þ†û~³?³WÈ%v›¹?·º§Ô>Þ?³àL'(0÷?é+Ný?»¿«DD†?Í̘°¡¯#?°;‡Áˆ?¾8ÐM'6H?¤ØžŸåN~?äſɝÝ?²à–P_?˹ìp á?¥î—ÿŽâ?ÃnÜpr›?¤Ô)ÁÃ?ä5Íß=à?­ ÂÊÓÚMIXED4FGL J1920.9+1408?ÄRßF|L?¢åŽå‹ŠÀ7ü֋'oÚÀ9¹°xÙ/²@µgJ0@'³Ù¶À?Ãe7'>?ÏxJAÃ@§~^ª°?õÉå"nâa¿×ÏVˁ?ïœ}^Ðoï¿èÉ5~'ñ¿é&$ÂW(¿ï9Ä6%¿å‹‰ $¸œOTHERunk2MASS J19210164+141003?¶ƒv'ˆ§O?¼ÖÃ'©ß"?»˜$u;|"?Á¤.bT?鼌Ÿyò#?Ç~®!ø	?œ¸ÄSÂÏè?¡±§¬|¬@?ÛÝÙÅ-Ç?—tù¯·?á+Lû8ùy?Áùú—á2µ?½"ÇG§´d?§Y€u?Èò`IÅ{?°•%a¾æ?æïÉØ?²±7‹€¨ç?yàÖëo?^l–ʽï?Ðk½ÆÓ?¦Å5˜Ûf?çÌ	3
&?¦ðݐMòP?¢YtF–é?²ýè[6?Á‹»ÞE£¬?Á·Úà"]x?êwyÄ</†?Äø+É*´?†77'Ì!ª?'»xì™Ôy?ßP¹Âj.ƒ?ÉM­Êu{ú?ßýŒÇڎ?ȯ³akÕ¼?´ï€=îq9?¡_s©<?Ç»QÈÕ¿?°mš›ÎÝ[?çs;±†ö)?±ãg¦©ãÄ?Y'Ì`—J¯?Fz'L?ÓXؐØÞ?³85O½äo?æG'-¸ÂK?³A	"™OTHER4FGL J1923.2+1408e?Ú)hèÛî¿ÝŠâ²_¤À5âœáL¶'À9t3poÔ¤@:'-ºM@Z}Sèµ?'d—·Ë?»V%¦'¶(@'•Râûã@É¡
&I–?ïåæä¦f¿ÌŽ¢…%™B¿á'r½Œ¾¿â'¿Asè°¿æ²*ŠF¿å[1Ÿ4c4OTHERSNR3FGL J1923.2+1408eW 51C?¤}K~rf?¥ñÉkÐOè?‰MÏËíš?–™"îoô?îSªÓílC?«¾áU?—Š".÷?¥lÇ伟Ü?ä˵ZÀ?÷?É4¯²?Ôïì|Ã?Ç0Þô[uá?Æ(C(|S–?²P }†»?´e¼$«R?¥nøðV?çé>þ?·wÎhS?vW}>3?aÃLô¹ö'?ÓÙð)Í?²˜Š`º¬™?åæXúö‰g?²¹¾ž¨ûv?œÒnˆ…t?šiÐÎñ–?"-zÓEŽ?"öcd¢m³?îȸ¹-f?Ÿ€'ƒø'?™Ç8©¸ÍF?²«"']Ì?äG#Ò0þ"?ѝ¸.§€?ÕÕDѧcB?Ïa6Ñ£KI?Ó¾Ÿs´i?´Ôê+L?¬¡žmXÅ?¢§Xê"î@?éPön ‹j?¸Ëf˜é°?[À~>ƒ A?MÃD9$÷?ÔÊ[êr¶<?¸1teÇHî?åŒñ˽`Ò?¸:æ!Zä?MIXED4FGL J1925.1+1707¿½øpKŽì?á†e_UPÀ9!<MŽ(LÀ:"*—ƒ>ä@ Úº¶ö@®÷ÝÏi?ó"»äG=?Æ꛿¹"à@®Ñ9C?òÕO[2¿ë"²Dx«?ïú|"eZ£¿ää­ßKÕl¿ç–Pn­\Å¿êäÞÚ4"¿æZêg‡OTHERunkMG2 J192501+1727?Ä-dßu?½ã¼¹•s«?Ȅb£–Ñ?ÅÍpMg^U?äØýXþ?É
ÍaOÙ»?¬L²þH ?³fêÃùV¨?¸ÛÞ«Rœ?»Þ^ßMG?ëÓTÚ#?Àú=>Á?ÆÒ¿7-?«¾‡žö?Æy_ˆi?­5ùÍfÆ?äƱä­ØÛ?²2T¯ ?µ-t#à§B?Ÿ3†Œ˜÷€?ªhn+ì<á?§`J¸Gö?ë³Ê˜ü!	?«F>/{?µaψ%ïL?¬Y›3Äõà?Ç'QŒ©_ú?ۖ§hô?ç‰ñ«~sx?Åe:ë ?¦`1÷|c?®Ô¡•Lö?Ækme¢àÚ?ɽï78"	?èÿ!‡³?ÉÈFÇõÐ?¹™k°‰=? ´8{M|€?Æø¹ž¶}Å?°u}‰kÇ?籊À҇?²Tï7ß)?¦¬	œ˜€?¢ÉIùÙ?¡`¼A(-?²‡±}¥˜?í?E?´9µËïÑ5OTHER4FGL J1925.3+3705?ê	Uži@#™·|¯ÞÀ;CØ>ð֗À<¹šû@ Œ6%«á?ÿ1ž½c£?зObïœ?¹Ÿï^V?ðRtý¾@àDª~ï?ïÿÅbu@¿ã+ÂüirŠ¿â`GÓÔ(¿äG@'‰?È=Qӟ$¿ïþæZ<ŒxOTHERunk1RXS J192520.1+370527?îäÔÞi,i?«øüʚ?Dó':"!?B£yٖ"?¡bjNðq?«t´ Å­«?êÙð2Þ?ŏÊKE×-?r'°Ï
ÂR?€rŠmv	û?Ç\
¸Ù×?Å?љ[?íÜ)È6¡?  p¯\ÒÓ?qµ õÔ9?vq*xCDŽ?²]Ĥ†Èâ?Ÿ*

̦Ÿ?ï¹È6Ç¥?f£Ý+"?0Ú«	!W?"qj
õ?<ô?fzýç	;?í²è"ú½?²b6í,2?Vřp·Ÿª?SR'8¬Ûr?²
¨'g9O?±ë¤R?ä·Íj?Ìœ"vý?zuàëuÒ?ŽÑì,Ÿ¬i?Õ¹#lì'e?ˌ&^þ?ë,X Lˆ'?¨?¼B5æ‰?{°í¡˜;'??¸?ÂqS(`?§Ñ#aÐ?GÓ?‡`ŵô—?HO¸$‡Ïù?E.XŒ°þ?žÉÊû©m?‡="œE²AGN4FGL J1926.7+3027?ÝRšš@¹èÄzÀ:•ùµc$À<UÛÔ§@xY W¹O@=áâß?Ô.ËÅeÐ>?ç|}T¨@LлnÖw@Ë#ˆÆ7²?ïý± žÛù¿à¬^YQ«¿é!¨üãëͿ웭p3T¿ï÷7ÿöšÑ¿ïôUªV€OTHERsppSNR G065.3+05.7?ÚÁñ¸¥µ?ÅÏ'(?ÓòùUۘ†?Ɓh=‰«î?ÒD¸kÁÅ?Á§}Õ:Q?ÕlHÓ$ø?Æڐ1K?Ñ[÷Ö"?Â7¦Šmן?ٌˆ¿V"?ÂJ©ÓE?âµÎÚä?±¢`$0u?Ê"/pÂ)?¬¶¹"sµ?ÊÒùY:Â?ªÆoVù+¾?Ù¸2(»?¤½Êó¦"?׉¿c†ì?§½1¤<à±?Í|}|	?¡wïG¢¶?Òì5VF?Ã$ÛNR?Ôý[
Jsõ?ÉIëï°Z.?Øü¸¾´"?ÅçþïJË?À@£s¸›?¾î[‹z?ÚRÝ4EyS?Ê3Ã"ns?݌Ñނ_?Ç&™qև?Ûct<<ò?µ€¤0²G?Ó¸úknÂ?¶iûÂ|¾w?ÐãöqXTL?±ÙÊiήW?ÁÅÐü~¸?žÌaTõû?ànI
(÷4?µ×ã"ÆöÁ?Ö@…gnµQ?²ˆ'+Ö´MIXED4FGL J1927.5+0154?ޖù]ÆÒÀèp—AÑÀ:Ê]†ÃÔÀ<-/à˜[¬@!ÞÓč¹?÷êSá(¤d?ÓûÒß5…?Í6ðÂuZö?ý[íœP-?@d¾Ö"÷ž¿ïǐÀI‡?ïuEâb`G¿àkbŸ1‰¿»<
rIÉx¿ØmÙ8>¿Ö0Z»¸RlOTHERunkNVSS J192729+015353?î£iè½'?—|¯&icU?ZÀdëÜAh?PÊ.súæ?¤ó^\ÜÊ?–ø@0+GÖ?íjC+_–?µ0q.bá?Sà§IÙ[‡?o»Ä¯LO?´^d·?¢?´'ŠCÇGU?í':Ö¦Ñw?›+VÜØ?s!ڑ¢§z?fµ%‹Îl?²< §gÔ?šk¬ò?î|2‰Ò?€tUÌ"O?bÔtÉÑ?KºìԗÚò?¥úôä,A?€6U°ÃM8?ëÝasH³3?³8óB°B?m0"Çž¡Ù?aՓXˆ@?À·àŠ!Š?²ùŽTƒ?è§TQÞ;'?Ɨ?S}?\äáÖÉÈ?lYò+ƒ?Í(äõ&vü?Æ{çl‹C–?錧…ëfì?¬éދ©%…?…­¸3;õ?yBº3EéK?Èr†g/0'?«õXùi®‡?컏ïæq'?—
ý¥¤î ?lÕtв@¢?b±G匬4?¹<ÔÛǸý?–ç?ŒîøAGN4FGL J1928.4+1801c¿î¥±I°ðp?ÒC.=€6À8½ŽwýhÀ:dÍcˁs@Pœ¹ʪ@>¤€}há?˔VúËë?ŀ¬"]M
@[µƒ+ß?þÏðH'2¿ï˜"}?ïÿÍgý?¿êpÓ§²a¿åÇ~)¿îÝ¡0fÐ?Ý»4‰tˆhOTHERunkMG2 J192830+17598?¿é,>w_?Á¿GÏ*(?¼È2b—"Ÿ?Á ‡)T ?èiÔ+Þ!«?Ì'Rš¤?´¤íˆŒ´Œ?µgÿÊV?ÁšÆærª?º¹a_E?éÞð"?À""a,{ð?ÃîåÍ
œ?ª…
â¿óã?ÈK(ñ!?¯ª\¯êz?äñ|PwU'?³œ¾ªœ·‹?½!à²TGø?šjh|áÀ?»¿€ÖKž?œ³;•Ó?èãÓÎb'á?£í›ž]vô?º#!Π¦?¾"Ë'€†?»–ä³s_?Đ ‰\õ?è·B™O?α­'§$?£':=‰:‹?¥SŸš
?Êo©PpÛµ?Åuy¥n -?è*ò4pº?Æ4™î0Ó:?¼"I¿U…?£âÿ0z°Æ?ÈbSÿ}ñj?°Ï•*ÔQí?æU	ö_(–?³K^<ÅZ? ø%m²;û?ˆ€æÓà•?Àð2`-?§Þغ'!¢?êï|mA…?©OhP©ï0OTHER4FGL J1928.8+3126¿âòYàWT@B÷+E((À:g²Û‰þòÀ;ë×!ºdë@Ô]ú@6?<Uñ¤?ÌÖ¬	2ٜ?½FÚ@9U?õŸf²¼€N@ðHäJlá?ïÿâ£Î¦Â¿ÐP¼{Eñ|¿íåmã2ià¿Ë'yꧩ'¿æ"9Pƒ¦¿ïÿ¸8º1OTHERsppSNR G065.3+05.7?ê-¶ùôº?»óBF:eÆ?ÿ'ŒW+S?‹§++ŸÁ?Æ)+£'À?»kçÚ«?è ºá¤"?Àúƒz"'?'y¬þÌm?"?Ì_Þ+?Ë-Þ×ޛ#?¾Ç]!C?éô•]l91?ª{^½r?šZ•,4á?¤õ¤N¬Ë?ÄâWãì¤?§ü	Ÿ¶?íYh2ˆ,N?Ž\ïµ:m?ß†ÆÂ?s"X•NxŒ?°üÜ»Ö{?Œ7ə1Võ?çÀ‰£édï?Á,?0!?Œ˜£8õÇ?‰€"v¸É?Ï4O?$Ðf?À»@Y¸?àUÜX0Ë?DZÎJ6–%?£djŒŸa?§¤"8?Üç¹ýè"¿?ÆUËñR	¯?ä
)ÞB7?²TýõP?±'hò¹™µ?¤ §ök¼?Ӂ'o'!¤?±>œâ"!t?è"&õ|Q?§fh#?©å9"ˆš?•Ì»»õ'}?Ç:á¤ÜT?¦¦JïøAGN4FGL J1929.8+1832¿îFVdvÞ??Ð=çâQï6À9i>‡ûÀ:x¦'@âdc¬Î@µ€šÅÄ?ù.¤"‰—Ä?Óf|`Ρä@`µ$9›,?ößz!8?îÐ^½$¹¿ëç?¿³‰°¿rÜHÚ~*¿çz
½É#˿胦³]þ¿Ôòb~OTHERunk1RXS J193012.1+183201?Ìރ×C%ø?Æ9Ë·½µÇ?Æ
¶Ù½Ãg?˯¾ÇÙüi?ãDñS¿Å¨?͸…nÎ??µ
B+K`?½dX¼|?®'Çì¤i½?±0xoÁ²?ëv+;©4¨?À1McúÀ?Í1íê:??¯'Š#($í?Èò"QŽ"?±«w\é÷?âvûñ
Úð?³D¦…âÃß?¸O¥Î&T?¦a˜N?–úTö?œ¸p©ž:?ì>;~]î?©ÞB×E?³?ÅӈŠŸøü?¿³kðdžo?ÆÍ­-±O?ÇÐWükJý?åªqƒ%?ÊfþÖy
?¬ê¨_5É?µ}bù(Þ6?²>4bƒ?¹úښê?ëéŽòÕ'Ã?¾Ü—¹"S›?Áҟõ~G?¦ý^1†?ÉoÛsó[œ?³Gm&Ÿì?å^Ôz|Y(?´aMv /Û?«¬Ç'aÎå?¯Å%3½³?"'ø<R›Í?¬¾a]¿®?í¨›Å÷N3?µ¤"æ]7OTHER4FGL J1934.3+1859¿ÔÞ÷‹Û¿Ýó‡·aÀ8̔<b†ÞÀ:lþÀdß~@s	%˜•ä@¦b…0V	?Éлļ³?Ớua«í@¦Ó0"'@ÖJ¦Ar¼¿Ô€˜›¿äð˜ÿjÙ¾¿ç/æw˜½Ò¿îvþdŠ¿×@Ъ§Þ׿ïÿôa¼2¡OTHERsppSNR G054.4-00.3?ÂR5—fŽ?¼.9†*ôB?ΉmºÌ!à?ÉÛ§¥'?ãÉ+sSè?Ê»¹@ËC­?ÇÅu7ô?Äå¾Fˆa?·­ZàñþÓ?±é9­àHa?ç÷VIsù?Áíµ-Qzz?ÇD¹så¼?­›‡–'©?Ç­&:§i?¬I'¡w·Ü?äCˆƒg ?³eڙKèw?°™æÕà½?' †Ø'È?ºº'Ipë?¢Fí+:a?ꕌà‰Ô;?¤¾×¿å ¾?¼åê¼21?¶"žLĚG?ÒvFŒ#?Ëà¡Ò‡?ãk;…3¨?Î9Ô9Jù?°*î2|?·bëô?»  ê
?·øáˆp§]?ê™kXé{.?»§•4?úMT'Ê[?ªömŸ´ž?ËÓ5EmY?±RüÜC"?ä¬]ò?³[Ÿ/ë?Œ{RL—;?vH¯ÚUt?ÁÚ4ß
u?±ÿH"1È?뎨‹
F?±ùLyÔþOTHER4FGL J1937.0+3003¿Ì/:­GmÊ@nJ82vuÀ:j´©ÀXÀ;®º××ÂÊ@ÌýÔ+»Æ@ƒπÜ3?Émõ¦à©ù?¼™:Ü?òŸ
纏?õù>ëM@{?ïþœÚñÔ¿Öz€5D…¿èў"•V>¿ì‹©¡¤ý¿ÙLªÓ}Àö¿Þþ®Ç(HOTHERsppSNR G065.2+05.7?ç&ÃÉݞ?ÃTz¥&"h?cä'oã?^<d?÷?ыþTÈóé?ÃDXßôÙ?å9 *†=?ÁÎ<Ç~?ŸÿYØ\¤¦?žTjK´oš?ӌÊ'¦?À6r˜Mê?èkïk¡þ\?¬Pâª0tû?t+c©?â±{袤?Ê­sËÔª<?ª{D¶;±t?èõóÁБË?Ÿ<ÉRýz€?6Yµ&]¥?'¿/f.7?ȁeÁáóa?œÖ¦µùÜ?ãtƒ\bÎÏ?ÃâõqöV?g³Ö'c'j?a"1Íî?Ø瑙ÅäP?Ã÷°üÕ?×`t	L?ÆÅN.ÈP¢?°Æff/l§?´e—YY€?â[ùNv?ÅJ½þÓ°?á±Æ,…Ö)?³S"!-ÂÉ?®=õ¢çŸ?
Þ‡b?ØÔ´ò)lz?²'͎é'U?ßÿÿŽ.ñ?¯»hxôºP?®+''î?›.¦—Þœ?Ü:›ŽÞ¢?­¼|œ®'ýMIXED4FGL J1946.1+2436c¿Ø8"±*.þ¿µê‡a¢v&À9ÖPfIàõÀ;1Cót×B@î«}œ¸Þ@ëø[ÆÐ4?Дr¾8Š`?ÛLÜõ)@¨>]2àþ@ìA‰ã>¿ïÿ…@ò
¤?ïü&âAþþ¿äIE=÷²T¿á‡n¾ú|3¿ïÿú Âî'?ê<—Ëc@AOTHERunkNVGRC J194625.5+243638 ?ÙÇ¢(ðu?Ä:ÎD#Ï?¬'–°†6?°RŽzÿ?áSID'ÞR?ÄÕpªä?ݦÑéŸÉè?Ï:Š™»AN?®åþ­1¶b?±ó¹l¨à?Þ|nAuë?͉؜?Þó"o?²eó&Eã?Âxô)]?©$x#_þ?Ø«©Õ½?²em-óÿ?ãˆPéÒl?°eÞ¿?ªÃœfAlK?‹#sÈZ¿m?Ֆ꟒ú;?¯<®‰¥6¯?ËŒ°cEÜ?¿ƒ»²"]Y?µCC%C?¶ÐMv/¦?æ'tp⍡?Ã.DŸIåZ?ÐF/(%}?Éؽ	Ïü?¼›ÈÚò?À›2ÒKx
?ä}	"ÒÑã?Ì`Í 1c?ÑË>ùv4K?°
ѦaM?É7@DNö?®ëv-€W?àÕR³3Ò?´EœõÍ)È?ӈzãSª?²Ïv˜GÞ?¶î}Ô²˜p?Ÿ‡ú#?ã^"‡êD­?µ€9Xá†MIXED4FGL J1947.7+2744?ãE Ä2õ?òñBè²ÜaÀ9|Ô4 ½À;)}œ
`@¨MŽ(LO@NU:Ä÷ì?Á¸Û=ÓË?ÐÂi\ƒ@Ö,wWOr@ý%­c¥í?éìjVµï;¿áÛÌ`ëÓ¿Ùp_ùºÂ¿æïÄH™Í¿èGóÐG¿ïÿÈ¢› ÛOTHERpwnPWN G63.7+1.1?ޅþ>+V<?Ápü<?·­éÚ:#?ª$
ÅW—Ô?Û´G•û?À¬Ð"=ËN?ҐcR4Ö?Å÷å'iÊ?¬—X±"öp?£ÔGx62ò?äîŠC)9N?ÆhÀõ©ª?áPtÃæ
)?±wÉ«©=[?·	ñÊ¡é
? ¼þvޜ?לš‹kj?±!ÀHsÐ÷?֓—Œe?¤ŒS¾v¦X?¶Êޑƒ^?Œp
xäm?áÜØfÅ2?¤ùÞ>>s?Æ8=çŸÀ?¸g´‰Óá'?Ì}çÎþ!Ñ?¾HþŒ"6?ãZ7üƏœ?Á@µ£ ½?¹ÄWGåqß?¶Ô~1F|?­÷«Á¼á?«Ïx•ìOš?êçú[†?¼rP¡Ðl6?Ñ5x¾"à-?±ƒm°á?À¡ A\m?§ãåtá"?ã<ۏ՗ï?´(æ̼×m?Âñ0ûº? gp]¨U3?¾Ñ´Šƒ¤?žy33?çi"mã]]?¨°*˜ËùMIXED4FGL J1952.8+2924¿ïPç'I>
?ðórS³À9‰"ç¨ñ%À;F"ÈŸ@£@iëw1æ@Hþƒ(?ÉçE³Z?é£opÑ#t@–¼b~?ü¯$¦}ƒ¿ë!ƒÞFqԿـaÉÁ¿Û"Êý¿³à¿ëÊ55kó¿é¥ŠÔø³¿ïüÚ±'ÝãOTHERspp3FGL J1951.6+2926SNR G065.7+01.2?ž@ÀµHhþ?–ŒŠüîŠ?º™Ì;ϱ?³4Áð>±?ëÊæÀé¿¢?µ7ßs
¯?­H"ƍõJ?±³Šl¼'?Ï ç3ÞÝN?ÂF6Ò»?æCDƒìx?Ãh8G3	1?Ðèޗ5ÍS?­'<
ìCë?ÌýèаÔk?¯Ð— "À%?àL€8ä<?±¯Ù%>?¶]ðôdå_?"d³¡ï?Òçú‰¸>å?¬"t"¶ã?ãÀDœDÍB?®Ëgý'N?‰îBŠ¶t=?'?LHé_ù?¿Š¹ÂYw?¶—/€"ž?ë¦ï½Š ?·<¬¯
-Â?—µÅ©Ü'?
†Ïˆ+?Ñ? 8U?ÅÅÃ(;ç?æ¢ÁÈ%·ä?ŮǓ§è?Âm(y]?§¶•Ó#o?ÏE®ÊÈ?´&x?ã"Tõ6·?¶K%6ÁM?–ϱ¿¼T@?~a"Í['Ó?Ör'˜Cå?»1j›?ä9%»{l?»& J/EŠOTHER4FGL J1953.6+1846?ïuÅòhâÀ)ùHUÚ'À:7ÁM<ɵÀ;Ë«¢°™@OÔS©Ë@ú37dñ?ÈÈZLQ½?Ҹ϶¤l@	ç™ÅXd?ýbG‹ÿ"?ïÿþÞ÷¿àiÒ+±^²¿ç©.ݎ$¿æ.52ôD¿ïÿõƒ¥;Ž¿å¡»§
›OTHERglcNGC 6838?èD†z¶ˆ?À÷úUu?§²9yx…Û?ŸïJKV?ÉW¶þ·ß?½¦å`Ü'¢?ß¿ËñÊL?Å2eÁ-ä?®;q^%Ê÷?¥®Ô"Ë-?ÜxÅâU}¾?ÄL§MŒOÚ?åqz¸û+?­ry'îtw?µEe°ä?ƒVŠIq?Ð{ßsI?¬–K×%¥?âžwo«?¡—
ëbÜ?Åh•tú\?šÅ˜ŠÌê?еD£|?›È¥¬€?ã¸ðE.?Äû†5[#	?²ÃìšÍ•?©£W|N^?ÓÝWzvyë?Ãbö¾Ò|ÿ?Éâ÷ÓØüþ?ÁšÜuó]k?¹ï‰Â	p?µBÇL÷?æcäß>?ï
QÕ¾A?ݐbßÚVß?±à–lvGp?ÁÝtß>Ù?£ÃpÍZÐ?ـⰆ<'?±õ"Ý4?Ñ7¯Ó±‡;?¡"sjüeP?Ó,‡Èa?ª1«.þ?ÛÇ;ÿÆ°d?§"ov îMIXED4FGL J1955.1+3321?î ̲±Õ@WŸß-øaÀ9ë!Ð4`ZÀ;U]"̃@6¬'=@o ×{|x?ȉº¾ØBw?ÔE,¥$'1@
yyh¡ª@	S§t£•ò¿æ±Q±£{›¿æxlâÿi¿â!?èÅQ¿å§ŸVqý¿è°ù'7}E¿ïÿýFKêOTHERsppSNR G069.0+02.7?íçÀð '?«y§'W·?€Ù²»]H?s¡G'1?­OƮْ?©Q"Éà"?旨ºb«¶?ÄZN(	¼ö?˜‰ß7?›°›Å—$?ÑN¶š9a?Ã
ZEŠ'"?ædžH2§P?±A.ŒÜý?¯•(ú'×?´)Ê°ì?ά¡–	¹Š?®ØڄíÑY?纤Ž•.¦?¢›AgèíK?'ïä
r?u‡(M|?ηŒ´-ï|?¢&°Ÿ'?ê'Éñ¦ ?Á¡´)VªK?¹¿/Ôy¬?AÐsº%Å?ù<Gëd?À}Wõño€?Û¦'Xš²?ËXORß²?«ŠÖáI
?²íú¦Ç!	?àtQþq×Ö?ÊX?ã_§t=?³—Êì‰?³;^Ò°6?¡©v¼Œó?Õ(ýŒ¢?²j
ñÜ·ã?ܲéT0É?°T;†ž"?¤V'Ž'>?hC}†¨?àaê¼ø?°Aê×ÿMIXED4FGL J1958.5+3512¿ã֬͆@J蹒]eÀ9ÀmzVÞ3À;"ëü<üá@ p8Zdz~@9{Kй?¼vY£Š^?smóÔ#?¿¹¶š†T@2õ«hN?ï<ÌQ#ß¿Ýüê6jY¿ãí÷¿¿ž¿Ú¿
|?k¦¿å"}¾Ùû¿Öh,#Ê_ŠOTHERhmbCyg X-1?ëDÌ>Ì2b?«
øév«Í?i½ˆç‰?[uÊÈ?ˆÈ
þÎÛ?ªÐÊs±F—?é@äY¹ãD?»8=–ò?kh"8?€Ô o8s?Ê«='u1?º™0܁ÿ?ëÏøk6.æ?¥Ú^O©|	?ƒ.×É÷û?v¶ì\}c?¿a«Âà?¥.c…?ë¿a¤àŸ"?ûÌ/™c?ƒ±DX#?`'®FK×?¿ŽÊLƒ«
?IŽidȂ?ä»4¾	?¼3ɪQ?'FK'‰?t4+LÕ0Í?Õ÷•ìøf?¼a¿/!Î?⺟t`5[?ÆÞdçW´ê?…Ö1D?¼Ûˆ¿f9?Ùáè°á'_?Ɲ´ú,V?äh<ÕHq?µÝÿO˜þñ?—ˆôÛ¤?†.>-?Öb ;Òǖ?µqr£*?å‹F?T~²?¤è:Q	²Ü?™3Rêgû?{Šƒ½™é?ÓP Kºhœ?¤XOÈüCïAGN4FGL J2002.3+3246?êr§ú|Õ¶?ñL] l‡À9u_€™"À:Ò;ߪ#@
+YuO@A\Á¡ö_?Â(ü8V2¿…®Ô5Ä)ˆ?Ãjt "?ði!#¼Ñ?é9Ÿ=Èb…¿ÞD­à#¿èær@U¿ê‹¼[f¿áª‰ O«º¿ß<À»ŸnOTHERsppSNR G069.7+01.0?àlïÛ«É?ÉíN¤ *O?"ëñcÁ¡?•^xäËϪ?Ýça2Ê؁?ɼÒ`4ž?Ӱо…›?Êà'+¬Åà?™S‡æ?›dÎË;?å\û…5£?Êڋ©c^?ØY<3"^@?³x0_»Ÿ?²<j2†Œ? ›h£BêÕ?á‹Ô |.?³x¯CÛê%?ÔÕ±Ô40o?­Àª¡¤? ¤ƒ´ãË?nýÚýå8?äŠÞ不?®_µŠJx?ÙN~¿3î*?ƶøê«Q?›WqÕ%#
?œz‡áQ?â~óْ?Ç(D_Þëf?Äáµ+'Í?Â7'¶:(	?žX@ˆÜ2?¥ò'c©?éÔùŽn9¼?Ù'l37˜?Ï!é›ÔK?­Á4HtŽ?±®!´,XS?Ÿ÷û€»è?æ÷Ï.üÃ?°+íá1?À'â^"?¥ŸÒϸgû?¦h¿ÞÏD?'²¢€Ó7?êt¾8,u?©•Ý*¹MIXED4FGL J2004.1+2517?眾RÇ´EÀ	ÓAü#ÒmÀ:}–FþÂÀ;0ñ9" @–—G"ÎÜ@ °«.?Ô5Ä<ÛR¢?à¯/˜sÿ¬@	)5ƒo‹©?ÿê5mË	©?ïÈ8éU™?îM]®±Ú¿á‡ÜmSÀq¿è¿ø¨ó©°¿ïÿáa¯G?îRý"ªúÀOTHERunkB2 2002+25?ÌUÁ[23b?¿±jp·"A? —bO?žå!*½°à?çáƒðÌ?Á*†Iۖ?ßvÕuy?ÅÎX¨¨J?¨
qgß'ç?¥aU"é–?݇Ü]8•H?Äp7þý%?Þ[çoÃåÑ?³Oí™Y?»£¹º²?¢ð9¾†›¸?Ú»PáÍm?²rFèáo5?ß}û>¶Z?¯\"î©?Á[Öð3§?¡å$T?Ø3ü\'?®3®XBŒB?ÂC:‰¶?¶ÚVdoÿ?°õ^5ÿ}?®7ÔÌ5þ?é[ÃoÖҊ?½9&I7Mì?ÇGÉ¢öº‡?ÀùôÁ;&Ð?³
šN¶¡†?µzvi*öU?çÌZMBAÞ?ÃÁ"!,?ÒCΞ*šU?°—Äègï?Áé&ë™?ªßlvE¸Ž?âcÏ,oìï?²èËü…[¦?Ë6^¥–—?¬"B¸êæ?Æ[[nC]+?±my{ÓW?㧌ÅÃ?´°îëÆ8MIXED4FGL J2004.3+3339?ƒŒE¤¹ƒ?ó#5#Î;bÀ82(1wqQÀ:'µÜÆ?@¨=ý;ª{@v½+o"?¬ Jžðת?{Èù-©@"ßGù"Õ@&†pG?í%^>#Ò¿ÔM€flÆ¿Þ®<Sme^¿ä?'Q¦»Á¿ê;Á!Gù¿ä«¢æIu•OTHERunk3FGL J2004.4+3338B2 2002+33?µŠMræ?¬'%³—?́È 8?ÁÐwÂ6?åìÍ&u?Âúêø/?²Å(8ýNT?¶>ôûr°)?ÎàxXßȱ?¾w°TŠàˆ?åï<⚥™?Á/ci¬8?ʔ܎"`}?±®>g'âû?Äù¿vDwK?¬§úONã6?äXþÉÊ?µ!§kO•{?½Û³"ý*c?•íŠÑb…G?ÃoY6—g?"{BÃ(q)?çh³AOD{? ›TýÚÍ?¢4å}ÝKV?–£ìBƒ¿/?ӗµ=M,?»܏|?å×uÆE?ô&§xn@?›äA$æÓÚ?§!7A½?˨(ÞE›?ÂçˆMI'y?è6Ó¿bß|?à gÒTÔ¡?¿><Œß].?¨—É×AH^?Èß	£ a=?³*áJ]FW?åàv{ü?¶ã¤èà²;?£\vÊøçQ?"I@ä¿ç?Ȑo¤S?£­| E¢z?èIJnýŽ·?¦%‰ÆJ¤)OTHER4FGL J2013.5+3613?š¢Iå}ýð?ðDq´xB1À9D5®7¶PÀ:ØÇNފd@È´p_Ž†@êC5öI?Ą‰bÙ?×Ò( °y°@zÒÁÙSÄ?øÅPt6³›¿çF3k¿Ø·Œž´`š¿á3€?ÖY¾¿çòøp¶L¿ì¯ú..ç¿ÚgzÍüwµOTHERspp3FGL J2014.4+3606SNR G073.9+00.9?›7	ô£êü?šXûå ?œë^¸×~?šU`ÜCU?î>îårØ\?¥Ì«&ÐG'?ÂöâuÈ?½ÜùÐo?¹Ça¾`ù??±kôENÎ ?è	[@öóÅ?ÁCéjMŒâ?Ɩ!ó¿?¨©uwÙÞâ?¿X3æ¿ð¤?¥'M¦ëä?æoqBk%?°`q«z'õ?ďeW6Œ?§0s¢OzÛ?´]mÉé	ó?•ÜAã8ïÂ?èPn-–Ln?¯Ëñ 7Z?'ýÈÈ£v?‹¢µ} ?›…®Œ73Ý?–Q)"LM‹?î‹êeJBÕ?ŸCœ8ºš?°<í"Î_?®´»ó‡?º—§•Êpì?·µ-›£N?ê¥mjf¦'?½NJnkÌ
?¹$³7¬=?›#Áöæîå?»Æ¤æ:d?¢Ê,ï®@s?éb"ü;´?¨Jn?ýÉ?­Ü9`У'?™r^Yú?·^é1(äG?¤1T"_{™?ë6_C÷Ž?®3Ó°ÛnjOTHER4FGL J2016.2+3712?í+Yy–?ñÝݖH¬AÀ9+RFòÀ:Syú—á@"5g+Þ*B@—|ˆç›?äßzÿ¥' ¿©ƒ—àÃ
?ô« b
·?ýRAüNŋ¿ÝGµ¡7?ï-.Â
Q¿ë€#¦Î5ƒ¿ãÛù%k¼¿ãKêN½Ó5¿ÜsZÀ•ÝOTHERsnrVER J2016+372?v/ô§?…vQ}È;?V43HŒÎ?jSó0ß}?ïÈ ´&Hû?ˆGÉ	¢)Ü?¼õ ¸i4ï?ÁA4Wsz?ž³–oîzr?£ö>ó÷,?ëk¯5.­_?Áà;Hî?ĎP­u³?ªHZ®1?±ì
Ñ.C?¢?5ñ®¢?èžÚL¾[?¯UÄ<6eb?²U*DÞ<?–/ò¥?y[±Jžz?rÝ !s›@?킣TÈ)?—'NÅ«ˆi?pÝànìO?u=|SŠÜ?QCÕ\³H8?fJ˜ßVž?ïÕ¢TºR³?~+5ð@V?´8n«Î2O?µpnqàˆ?¤Pß1ýsÌ?°.ÊdÇè¨?ì3ä7fby?»'W»[hå?¼ü;³Æ}?¤C#é;·?°-tÝl?¡C&¹!"?ê_›òöhc?ªÅ¤€Ñ—O?,Ci‡D?Ž7bz›?k¨€~ Ýñ?rX
ÞÕ?îúõdE¤Ð?NÌy'S"OTHER4FGL J2016.3+4953¿ç.mÈý­@ ;EkD¹À:²€	¥›0À<`
šó5í@!èÀA¤?ø^h5sT?Îë``½Û?ÊO'åJr?üôÙáˆE´@XÛ¾­$f?ïðKAœØh?ïÿQ"W6?δ°¨©Ø¿Þ'Í»à¿È%6Æ:·a¿áБb"sOTHERunkNVSS J201619+495324?ëB!Þ;?Àqø7V%?um+q—£?wˆÎæ•?ÂL"R=ö—?Ày_ˆi?éã$ëíF?ÆQÀo¤Ü!?yn_âœJ'?Š|ƒ·™¯ ?ǧùT{h'?řûÔ¢.>?ì° "¯O?¡ækI*Û?xkíìöB?v3'_?¸ôO>¶Üç?¡ÍÃ0°Æ?íÍI›™<ì?Ž\Œµt?y–õ(¬Ð?f­K#~-,?¯ø‡¨ºÐŸ?·òÕ]?æ"
."*?ÅF¿«?Ž/ú_%V0?‰‡a˱v?ÒÊl
üC™?Å;¹QùO•?ãõ*úÞ
À?Ì<ÀÇþ(\?ƒŠbX˜Ð?"†?×yVø#+˜?ˈ§T©`È?è	ºF~¾?¯ŸHGPþI?‡\ƒ5?'?uSò£ÿ'?ÎcN³02g?¯¬qê?êä·;ãRm?§Ø™Ûú?ƒxÄÐꔺ?w²$ׅ€?Ã5–ÃYB?¦ªE6¶€AGN4FGL J2021.0+4031e¿î"‡!®Ó@'âûã:ÍÀ6ûî'):ŒÀ9ºG²F8É@!ë$ ?ýþ«×‰¿1?¦ÙÞÃð/?¯BþñüÌ@Dnœ•Í\?ö}X@?ëIÒF‰QM¿êPãèrDÁ¿åŸ£i&4G¿×Mn]UƆ¿ÜºQ,k¿ßŠoŊ¹,OTHERSNR3FGL J2021.0+4031egamma Cygni?"ÝÒôþ?˜.~Æï
 ?s
¸'"¨?€̓±Ã?ï:û÷\ÃO?œ¾þÀÖB™?µšþE+2?»ø³õ)Q!?Ñ%uŒìY|?Êm^[!†?乑Ùܪ»?Ê}À4QÛ?Ã%Í­P
g?®ìfŽ2û?«pÿ¦Ñ«þ? ©³î©-?é|šZ^Æ?°Ö¨7ªé?ˆ3˜"Ôx?r†E÷×w¬?¥J®E•cê?'ëÛÌ=1™?îJ†¹¡P?•kïuÞ?–3¹ã2Œ?•klý²²?p­	aøHt?uµrJB??ï-¼O7[ó?˜š±QCP?¡•J'ÇÜ?®],H5ã?̼¯¨úŠ ?ʬf²³éH?ç·m?ëË?ʐ§ESÇ?¾ÿR8º?«`r'9¼Ë?¤Ùg7b;
?™Ó-ÌÝb?ê¢ú
?®ât¢ö?p'Ë\ÄV?asAªÀž?©³'¢ï?™žnŤr7?îOÍÀ'¬À?š'÷䜅OTHER4FGL J2024.0+3202¿éÚ|λBÀ	,ºËCÀ9Þ Ž€`ãÀ;GµöâJ@ {¼ý@Á…pí©?ÈÚþ=Þ?¹E\U–_}?ö8N%'ö@"I­/?ïåÑ0é­?ʄ‰§‰r¿ä™þ³ú™¿è'9
gǏ¿Ì†£V‹}¿ïÿ¶ßO±COTHERunkMG2 J202410+3203?çá1Åí,
?Àœk8»»á?ZôSêÜÙê?PÕd.Ög¸?Ð"¨ˆc?À"¤ÿu¹?ãœðÍÌÀÒ?ÇNíÆ9K?}{f-â5?"G Þx?ØP0Ìs#?Æñع®Ñ©?鈖#ê?©dwX9?…|^ÓÔ?‡õrɦE²?ÆüÕNâ¢]?¨—ê¸c±?çÑ,T¿x?¤'ÎPêÚþ?~líV–¢â?g/AQ.?ÏÇçCàCf?¤e*¾Ní"?ÞBÖ z?Å
œAk°?pN=e¿4!?dÇg¡9¢?à½ø4ÉO.?ÅK3…¤?×s7kb_Ø?Æ/gºç¿?—½û†?ú0[ˆ)?äYM‰ ?Åٓÿ·a?ã"oOƒ?µê8] ŒU?›Ïgóô?'rÿ$§e?×:ܱ¦Z?´ðïƒëcd?Ü+Bÿ.ö?²¢gYN§?Žv5'(Ô?¯¶_L¿•?áp†o'¬b?²ºö'èfMIXED4FGL J2026.5+3718c?å¿\+"¿àЧLàƒcÀ9½Í!†b…À:ßöX·Q;@ÔÉEƒÃ@¥
ÙwÕú?Õvzۓd ?èfÃî×¹@
me¼{a?õ°r‹ã£~¿äsþÔV"¿èªý¤Ûìû¿Ü`wIJ¡þ¿îø‡›jT2¿¾_~8j*¿Û•Ü
Wq×OTHERunkNVSS J202726+372249,?Ð0ö Çå?ÇÒ¢]:ï?¡› :4¾ª?±i$ò•Ã¨?æÍýu‹r?É~ŸôÂ1?ИY½æ?ÈÖÅIُ?§=a4"?¦aH<¬D?æ@-«pú?ÇÁ
òµ?ՄĮMäB?±Xîî/ª?½I@!‡-?¦P¢"j	ò?á"u¥@
Y?²	^¤USQ?Á`'æþ8?¥TZS?¯ÜÎ:ŒÎ?žÊˆœ=°1?骉lU?«2-•2®]?ÇY®c¿?Âwš(¾BÏ?¥Øw·?¦žW)îý?èÙcé´d ?ÄÇFًՔ?·îE"O?¹ýºf©éY?¯7}fY½?±‡
Éþ?ëÌÿw™ê?º£*–Ek?Î4J±h9?®!ýŽ
'?Á= ûUÔÑ?¬Ìß¼õ‡?ä#¥æ°½?±ßzÿ¤á?N|D1"Ü?‹,ŽŸÈ?³ÚUXnx{?¬9Làó?ìšAr™®?¬ì—Q¨KOTHER4FGL J2027.0+3343¿Ü´=-"jÀ8''
À:u¹Èä
À;…-RH¢0@#±"™ªŒ?ýgQbÉ"ô?ÅcrÁ¯Z¿®—Azž¬©?ð'¹M"‰?ú'Ÿµ<O¿îy`^dL?ïÚ­`ûH¿ì%V¿ÝÀ>Æå,¿àQù\wпá6—Á¨+ƒOTHERunk1RXS J202658.5+334253?Ï£¡ôî?ÂéKјA3?Rú«ÍìÒ?L4š2?è1æ0 .?ÂïñØÜ?Õ£#í+M?Îqásݍ?"¦+ð–"
?¡¿=1!?äÙ}@?ÍÙ "Úy?áK}MÍW%?³×´îoðå?'p_•e"?Šä¤à»×?ÜOþ]Ç%?´='0y"?×-?úÓª?µ<7‹)? ­<ù*…?'%5iz_?ãiU.¹."?¶_'ÂŒm?ÂáŠît×?¼Þ"Žäùƒ?a&î½®¤?[Å®Œy,]?ë6vU‹'ˆ?½nÊ/…÷?Âm×Íß?Ál6ò
,?˜¶jàžÏ?±çÿ&î?êžå3~1?Âò<;*à?Õ1æ#']Š?²VfüÔËv?œV¨'•?ë{õªø£?ä"\1?yN?²'!ÔwL?À‡Á ?ªXHôïj?¦^"¾v8e?¤Ÿ^ì©ÉÙ?êxOSò'Ñ?³¿F>AÜMIXED4FGL J2028.6+4110e¿ß<Âݤz7?öW¾VèDÀ4–š9ŸÀ8¼ C@ZgPœ$¹@wkcü(Û?…kŒ.æ·? ¹L^ʳ@¶Ã ¢@wu2)ô?ß&2dZ™¿Ê¼˜·œcù¿áÔ<iÌ¿á¹n¡q€¿âqPÚãæſޏ¹OTHERSFR3FGL J2028.6+4110eCygnus X?«tH+†Ï9?¾Àê"\>?ƒìw·òu(?˜Mcš‹v?íù	ž0Ïx?¿úÎIÆêØ?úOUÂn?ÌãUFž?݆¬è?Ó[ª3"tÓ?؜+lä1?ϾÜBÐMú?ÍzA¼°As?°
ÚS¼ùB?´3ƒüü?¥!W©å5?æ‰ ‹Ìä?²¾šM"JŠ?‹mÊ0¯-?€S§Â˜?¹úN …—À?±Rp4ºT¢?ìSÔ¸ËÛ?²Éòpk'?¸Úï¼Rª?ÏÇÆeù?êf5vt?®Pýêï%&?ìœøp‹û™?ϵ¥É}·ç?´,"íïB?Ã9¼UAŒ#?à±*í?ÔAŒá¿?ْ†âª&&?Ñ
åu©ê?Êê	bn#
?°2ê53+?°hwùæÕ?¢hšž&q.?ç1ИÅor?³zNsØ?}w¢JƒŒ?sur—m´?»¾¤>c=?·ÀÝùÚqÝ?ìMO¦ÜMH?¸Zt±%þ÷MIXED4FGL J2032.6+4053¿Ò¯E'Ü;*?äO\"UŒúÀ8ÉRÄÈòÀ9ûtä®jâ@R
b""Š@´œU5¼?Łø4È?ÔNžÃO @óíx:¤@¨×Ðâ¿Ô(v;©Ï¿çIüm¤HI¿êêgèF¥×¿è–Ñ"qïÜ¿ëÀ©s+pÇ¿ïÇ/¿`R¦OTHERHMB2FGL J2032.1+4049Cyg X-3?èk"·¤
{?ÆLÛ.\?'XÞeø?˜_¸ºU­°?Ì&ÑT_Âw?Åò³€r?â*áÌÒðÂ?ÑöǚçU?­üB}¿?µÈL聂M?×ê´#ˆ›E?Ё$Œk!¦?×8Ò¦Í×?³"Ô:[Cé?ÁŠ¿JW?«:¼ÞOþ†?àæÅFp¨?µPß)e?Ô©‰gXõ?¬ü½Áœ6?¤<€ŒGð†?‡ç;Üü¥?ägsCeý­?­‡8åls?ßÃéã,$?˦——>~?œ8Ւ Üø?!¢c­ÿv?Þx‰š"6l?ËÇ·âãm+?Ö¨³vÿ)°?Ñ~y^?¼ŒÜ
Ç$?ÃÅÌþå"?á
Ã'‡ƒ?Ñ$d¼uÅ2?تØG¢£?³¯`ð/?Â}ÚҖ]?­"-È"?Þ¥aòí?µÏ9ùöу?¹§"!=E?¡âH՞çé?²öÆû•?›ôòî.?êlLØ(~,?¨$<C~å MIXED4FGL J2041.5+5554?µ,Žqr@ é$Jb#âÀ:Ù­äÀ</êp'@2=²hŸ@^´UªW?Ð?ÐDÑkB?ÌÔÜeÇ6?ýeuU²Ê?÷ …[Ÿ
¿Á³k¢Š?ïäÂAÉy¿çL`RP¿ÞCиò$¿á!Äuæ6*¿ïÿîÝÃÀ	OTHERunk1RXS J204129.4+555144?ì—[†	¢?­þeBœT+?€¢ê
€N?y'öÎd7É?¹AÏrufª?¬x÷ò<À?ã÷ÛÚ9z~?ÆÝ¢™-Ê?£MUÐu›? áp‡5½?Õ¦'S''?Ä "0?í4O»)6Z?ç.Ÿf?'÷Ë?"¯x²ê?²»ñÇe×6?›ŠŽÑÎñ?éér=›R=?—t"#('(?ª•ß´j°?ŠX78KW	?Á´¿Fɵc?"[&`I¾P?ç>í×g
3?½TJžÎ|?'äà9È?‰dSÀ9?Ða¶ÛÒy?¼-|(ß6?Õþ/؂/?ÅBB–
Ú?³Èö€œ¿á?²*mªä?â‡ÉCf˜L?ÅYT¸œœ·?é+7½AЖ?¬É÷]Ù ?¡'׶
WQ?""ž
¬&?Æî«>n?©ÊθèÇÞ?âæù֒•¼?¨€­Xv
_?¹8¤8
uz? c­1M–;?ÓããD2‰ë?§²®¨p1MIXED4FGL J2043.1+4256c?âŒ&ª	?Ô[Ý¡[YîÀ9;αð¨À:i­°hé@¤S³Ü;@O¡»§
›?×¢‰G;ÿ?í~âÿ>9!@Xt »ÌÊ?ü»ÞDno¿æ›å¿ê¿ÖO© ø³…¿ë}Žc|¿îÛ-M@$³¿ïӘc8´|¿ïø~a.ïOTHERunk2FGL J2042.0+4252cNVSS J204232+425813!?¥F<Š«ÝA?«KôÕgl?¡RÎ$­â»?±Ò+FÛ?í–oTîç ?¸ÃÙ ½Ì?¼{çh?À›?'ïžä÷?Ë/âªjÞ?Á(Z©¼õ?夻ZÖݔ?Än§
ܞ?Òáíf±v?²•ý²Å?¬š
Ev?©Ì{KÙ?áãâǤ³˜?´	\6l
±?•ñÀ"]¯.?v~†Ð·—?Ôý†ì]Œ?²œÒ/`‹s?äÑ®÷'`¡?²¹é"vCj?¡ä '¦ô?«‡žù¸¿?¡UÍZõ?¬çF%ÍEÎ?íÑ\Á¡ö_?·.<¡*Žr?§H\jX?´ˆÛ=¸N9?Ò¿¹=ù¶?Ë@(9/!?嫝ìÔC?ËSÁW<–£?Ëó±$?°')Ò{&V?ÄèÌbë!?¬	ìFr|¶?ä§o?´c‡q2y"?pî"S~â?\à7ý	8?؜`d(?»Þ,ÊÓN?ãòËRèõ?»Ë:;J¡OTHER4FGL J2045.2+5026e?æí#b
o@®…bªðÀ6ÿp·ù1À:wÖåTƒ@¢¡Åâø³@8¿E$Í?rj֍•Õ?Ì&ãÚ˜Á@*è"úô'…@dk@?á?Ä/ZöñŽx¿ÖËF…¿å‰·~±áº¿çÏ°!Etÿ¿ïGšþôgF¿ïܛ¬™PžOTHERSNR3FGL J2045.2+5026eHB 21?ŽcHvQÆ?òeè±­?è
‰N{l?Ë5Bßçº?ΤôÒ·?Ê HþK ?—.ô½µ5_?¬,Æ2«ƒ?룅ÔüØ??¾QŽÓlùþ?½&†/7?¼V™âDÏ?ŦZ¥Æ7?­#9$•´Ó?á†	ÔaŽ?´ÉN
Àq?Ò ¿Y£W?³kh¿AO?·Ue»ÝC?l"Ëú>õß?èS&±MH?¬`P ÷õ?͗ïâóÍ?«ÄºáM?ƒe‹)|@¼?'°¿à´?éo~¬>ž?ÖÃìÜë?ɬ›ÿÐZ?Ãr&Á"f?'¯ç+ SØ?­\§Üœ4?ìã0üñ?Á"È÷LŸ?ºÌìµÓê?½cNÑ@Ç?Àɒîã*»?ª60
s?⇒or˜h?¶Ò꿙6?Ҍ©©9Ó?´êLa…?d€Å‡Í?Tpâð•sÙ?èFQr…ÐÜ?³gòÎ+V?Δ· ïs?³tÒŽÝPSR4FGL J2051.0+3049e?ÑÞ­1HnÑÀ ìµ»8OÓÀ77Ú¼y˜rÀ:Õçd'ÇÅ@¡ÓÏËZ@ž¸Ø#B$?˜¾"ºêø?ÉpÐãõè@-f8Éu)x@ˆÇÕGj?ïÁ´ †å¿ÕL@ËLD¿âßhæsg¿åÛ¹™ê!q¿è*'ò"È¿ê†Iàô¡þOTHERSNR3FGL J2051.0+3040eCygnus Loop?°JÆúÈ*?¬sZí@Ȏ?àÒFä•ì;?Ïihàze?ÚHÀx«b?Ìsu҃߸? aÑY¸þÆ?©	
I¾¦?꬀	-XÜ?ÀÃyk?­Ú?Á5‹ƒ''_?¿H2Uµ
±?ÓÃÏÎ	
?±…°ñƒ?ÖctWÐ?´WûSBÔ-?Ö|È*Ú&Û?´vö†?‹´}ÉÐK?wìànºOÌ?èRæ…Á²?¬Ðª2·?Ìú°ˆ§¦?¬ÐXçZ"?©«Ö&û‡ï?§É~Õò0!?ãŽO "–?ÇúÍjpP?Õ­ç6?Åã‡Ä"ÿ¯?™mN:Š:b?§u1fq§w?ëµ·–¶?Äz'ÅÔyÙ?»ü&¹t¢·?ÂÐ òÇeã?Ï8x¨™x?°ÀõyÐa¾?×w4z)¶?µÝ{÷–PÄ?Ù¯I¦‰?µïò܋?q‰ž¤ÆHy?e5P¤r7˜?ç'C4:ͺ?´
ÿÎÖ?ЕS÷Kj?³ãûÕöWMIXED4FGL J2056.4+4351c¿ï÷€ññ¹/¿ïDË ¥<À8âô2}À:¦"%¼R@ºvQëÛ@ûB+»?Â)Zl] ?ÓÆ¢[Šk@!w~¼ž?ø-c­úN»?èáºÅc¿Òô&­é²·¿åá?(‰â¿ë	ë;LÝ¿êåB_ !¿ïÿÿ>¹úOTHERunk3FGL J2058.0+43471RXS J205549.4+435216$?¤$ăȹý?¡ÀRÿ¡ùI?ǞÏäY[f?Àéݺìâ?èÕÿ¾' §?Á8â)€Vý?‹ðï@ë?½(+$=nm?ÃÓë9Ÿ]ÿ?¶C§•µÓD?æhõÇíÀ?¿qʃØxc?ǔ={ØàÏ?­;ÒG˜Âp?Í4°ÿÅP4?¯w½ê›d¬?âÍÄas¿?³BEÐOÖZ?«,ù[y?ˆÅ±ï^™ª?ÉÉìCpÔ:?¡1È9•"?çÚďÅ
?¤åá17ú?œg¶ü­+?•‹Þ9™{?ÁÆO'ý©l?¹4»ï¨ñ†?ê«.g¥k?»Vt°ýq?¤­–[«?¤S-»¯V
?Ã%ó±µf¡?»{×"!y3?éöh:º}?»]Àe
pÇ?¾,ÁHŠ2?¡a?¦'7?ÎL"\‡¯%?°Øs`T;‡?ä§X°+''?²GÑÍÀý1?Ñƒ|˜a?sž5¸Y/j?άŸŸ~F?¯u‹73É?çݳ‹¡øý?°0ԟ?¹OTHER4FGL J2058.7+4454¿Üfž›GU¿âçF`6¡}À9t— Ÿ³À:þºoÒö²@«œÂ˜ìK@7á2µ^ò?ÐÔbãz
b?ÉH±õ…þ‡?û}E‹$‹Ñ@P	N][%?ì¡ÚƙØ?ÝjùÞ}Ï9¿æˆž¿É.2¿ç»Sþ"Õ½¿ïø*~XËs¿ï–ü0g¦ØOTHERsppSNR G085.9-00.6?䐀38‰?ÆOQþ5¶¬?Ÿ.…®¾
?‰²Ë›~´?ÕÕöZí?ÅÞ)<Jš>?á{ûæÄJ?Éö$a
ÿ?'Ÿ›[þ'ô?'û•.CÀ?ÛÞ~^?ÉX#[éy›?âHUAÒ?µ¹¶vzI?¯õÔo?œ©àé®<»?׌7\sÚ~?´MÙ Yw!?äˆ3Η/å?«ŒØ?A•i?¤¯Zô]Ù|?'ªl«»?ÔY­ónf?«€:Sâ ?Úó±Æ"­?ÁoÝóæ—#?•¤ß'>?£éè%—?âLß.y:)?Á¢"¹y͐?ÓÒw\¿ó?ÆinKÀ¦V?vîã}?¥²½T.?å+Êg0«?ÆÍ)ºŸ´Í?Ù¥v(¥d?³Û÷ë'o?³c3ûsíý? )>á¾Ö¨?àÀÞl‡g¾?³¬e‡Åæç?ڜé® Ö?²ðQDíÐ?­&ôçO?"÷hi¼U]?àßè؊à?³Åøl"§MIXED4FGL J2059.7+4837?ä2J9¬k{?ûF8Éu)xÀ:º}SèµÀ<T«@‹
‹@ÝÌÃèw£@‰à¤&?ÔÔ@ƒþ¨?îh—c^t*@¼8zšÐÑ@ªæ:²œ¿ê`ª?.>,¿ÞHšu%F¿È¢]b†²â¿Þ¼£¿ïý²6ci¿ïºýÂcOTHERunk1RXS J210008.1+484122?à=©+¬?ÃUáÞ×¼?Ä9ô…ý$?µ>óP‡;z?Õikâ?ÀÜVÅ+E?Á€[‡1¯r?Â5¶Œ)Õ£?҈q@ëO?ÅãÚãÄi?â[°'|?ÅåÌò{Kê?æ
8Wgù?°mp+	?Àt¥ŸG•?§wöGÁo?ÇUãy†?¨ø¸¹Ê…ƒ?Û2‹}¢B?³=ÅVû~*?×P©è¾'D?´eÕp*!¡?Êù•3>¬õ?©a-Öø«À?ÓæÞþŸúÿ?ÀnÈôR?ËjGJÜ?¹è'Aô}Q?Þcý]à1?Â&Õ{`ã4?­Ò€ç'@ô?³]¨ç¨5ã?ÕëUs¤èW?Í#Ŭòç¿?ã--7úõ?̄٨Mä?ßòY¤ë?´¸•'ÛO?ÉX·š‹‡?°âÀ0 ?Óa÷"ÙR?²
ð^›m?ÃÆ£tÜe?­ÚƶÂ?á>³w™È?¿÷?3"ù?ӟGV^d?ºhÛ$˜)œMIXED4FGL J2123.9+5158?î"Â=?óhG7À9ó¼¾aÐÀ;
cûRV@¢ì1l½@¡¬Âk?ÖzРìÊ?á›Ό@@@Þ$
%'@5òzÜ?1¿í|ñýþ?•·©=ë6ß¿Üàû㐳—¿éѺ¨¿ïûR}ÔA¿ïqNŒU
yOTHERsppSNR G094.0+01.0?»-^®?´h,l`¥?§º¢Û?¤qP2a?ë*#N±
q?·ù…H›þ?×'¦]?Λ«ö-a?±Â¤˜'?­"ƒrøf?â4=©{0o?Íd8ˆK'N?Ðüù[²>'?°[ë :2?ÂxZ¾¬<x?¦åŒIq?âãl¢{љ?²ñaZ!¯^?Õ'wmŸÀ¥?¯…o{nþi?¯8ø{ô?Ì؜tüh?ãx´Á,†?°êj>"ª™?¨X¸a~?­µwŸ'?¦',¤	l?¢íe'<?íQ¬ÎˆA?«›v²v?ÅW–²çüÝ?Ãt—ª^Á_?ºP[PøZ?¸²Nl*¾?çi°GÛá¾?ÇF÷ôvg™?Àµ.ÌÉ?£{Â4–«@?ÂDvk[?©<mXBî.?çP‹ã¶?°Ûä-*t?•ˆ[r?§MMvçy2?­Ìyíû?›1.ÍÓ	?é}ÖWî‡?¬ö©DPt´OTHER4FGL J2129.9+1208¿ášSâÄõ'À;Q½aõ¾^À:1'"ªLÀ<5š5 Ë½@í§°³''@?"äMòÒ?È'amÙ!?Î!µz@OjCj¸Û@ï/1?¼§»rÈ¿âè
`+8é¿åo‹^¿¿ìò_c<æ:¿æoA×:å¿ïÿ»!(ĚOTHERglcNGC 7078?ïÆ1,ÂÉ?|À´›<®Ê?Uó¹hF†f?U'Bv?wj{Z|•Ø?yõ FÚ?ﮢ4Áq?ùœãÌÕÈ?^éC›KM™?pFùˆÊmè?€zJX¶?z¯aûBº?ïqEê'Qô?"0êZ³?rheo•?v›'=ó?ŠzR¬u>p?€PáûxRí?ïZjÐêyí?h}[q8?k†|â íq?Iòá©áÝ?'AÖ>Y»?f|¦«;?ï'©ªUK?·
¦d`Û?e¸s»ÄÕÈ?c¦Q=×?Š¸¢ùÔ?Ž§@WPL]?zQ?™æ#Ýk?tEGpØü?€x'bVñ?™.'`ʤ?•2ªHÔµB?ï'(öˆ!?t"®P¾g?}ê;	ÐÀ ?{ÜD†d*?˜SLÞäÝ?Šg;ob|?î7å8ö¸ü?ˆÉuI¼¦?€˜ÀVuñ1?jÜw,¹ÉÉ?¨[|["îö?…ëÌx[^àAGN4FGL J2217.5+6346?ïæ`:ìÿ·@7hiÎÑÀ9Á²'ž«QÀ;ÆAÖd%D@!	ò«¨?ý顄I¦<?ʊ¾	w‡?Æ*"ÿ%À@I"¹`~@×èØñô$¿ï{ Ôvd?ïôx½«ò¿å/ù‰¿ÛõsŸ‰ó‰¿Ø§–ýˆ•¿ë?o¾ÁÇOTHERunk3FGL J2217.2+63461RXS J221728.9+634714?ïs0­X#"?‰…4£Cé?CŠJK+GÌ?<¡ý¡B›?ý˜û?‰¥îÝ?íâeEí©?´BDÃà\?cnv'
?s#µN<Ë?°TDa(<?³h²ßÐZ'?펴©ü? dðÖ¨~ö?'ÂÑWT+?€Yæ|×-?±6°0jô?†¡"dց?íöR½Å¦p?…´Óˆˆ?€ !N×n?cv|NQ<?¬'Ëиx?"Ú»ÊÖX?—¾ðc?£ÍNËËY?]›UÍ78û?\€&Úøó?¥‡ë׋	?£ræ<傉?ê°%¦úø|?Ä
¨>fÜÈ?yõÁÆ[
?‹I4!PÏÕ?Äo»U<X²?Úó¬	³³?ë-ÝçYô?©kÀû)ÎÓ?'bÙCF´l?ŠÀ)ºU?Á'í`ž®à?§ÎÝ"…~?ëBGU²î?"iȵTÐ?{è€Gé?Â
65zm?ÀçfÙbé?ž
/a™,tAGN4FGL J2219.5+4653¿í°)Î?,À ÙXS~,VÀ;W«p_À<ˆé¦!gY@ Á"ý}™´@ÇÄ\»Â¹?ÄÀ¼ؑ|¿«å'²¶?èåRŸà¸@œw!ŸŒù?ïþ~ö€$~?»Ä‰1l‰–¿éXޛ¬C¿ßêÙþ
·y¿ìŽ°Ëæ?åÄ #!OTHERunk1RXS J221919.9+465137?ìY²v6"?³øÂQ§E?p®Ëªëd?i'­ó]¥6?¼'ƒØ÷±?²À~8ÁÇÉ?çjtÚ\$?©FþÊ©e?{¯Ä¢èh?†£ŽÙ©ð?м[ÂëÄ×?Â%¥g>cÏ?í
´?¡I[P¤+?†	B¶îE?'h#£õÈW?´©5€Û×? Nã0?î§2rTA‡?‰ÊÃÉs?v£ù\¶Xÿ?`˜]:ŠîÆ?¢¸Y­ƒKó?ˆéøLo~Å?é`¼Â#â™?¾B€¶§O?|¸‡_Š?vj.Ôø?ɗLڛŽß?½óÒ±N}M?Þã'û´…?È6aŸñç'?zë£K!þ	?‡ÝX<*s^?àX_;"˜½?ȃ»O»™?êZÐýË?©ÏqŠ	m?Ž
2²$—ô?"´¥ÕºL?Ä´°B†?§èbÝf"?ë‹9œH?¦+´™Y'?'JìZ­?ƒš8]6?Á|Ñ^
?¦©dŽ†&[MIXED4FGL J2241.9+5729?êY©KIñ¿ñÈ÷ŠæxoÀ:!´¢3œÀ;"¾â(@Ûé	ïB@ðæ[L?Ïfr»3rH?ËÙ©T!ÀD?øö
³¸)@¤[›(¿ïd~š9Ҋ?ïþÔò5<"¿èӐÁê¿çŒ>'Γ¿îò-Lie?Óª¿^UKOTHERunkNVSS J224154+572700?䃵r¤H…?ˆmRÏìÎ?"¼Æÿµ*º?'ÙÖ#!h?լȪ/
?ÂqÔ¥fà?æÊO%pì–?Ä4"…Ïüò?‰fôú1?"#)…zƒ?Ñ 0Ìür'?ÃåGB	?æD:¨?°f[—?©À—q?–"C}dL?УŸïk¢?­~¥:vC_?ëø±ÎTó^?–¬†<aށ?™jŸŸÜÃ?|"Ómœ?¹ßÉ¥a44?"$ˆsÍ]?גTÁMg½?ÃÒ²…ßä"?«7ŠÇùç(?§æõßR?âƒ\ó9â¿?ÄWXA	µ‹?Ýϯ@Ûùw?ÍzÈ*,X?›êBÁ€?§¢§Ö»fˆ?à?w°væø?̵4E¾z?ÚM¹,˜ ?²`+¢"Ý®?¸ü¬¯
-Â?¤&s±Mvs?ß¾‡¢(ð?²EfÙ¬Bä?æhU¡ƒ?«æÍV™ñ'?«
F?£…¶?"Ý›†k¯õ?Ï7n«F?¨)ö¿&«MIXED4FGL J2254.9+5802?׎Gmx²¿ö…È̍íÀ9úùXF3À;œØ_¨D@çõ±óW¦@ål†;?Æ5Ÿôým?½ó"Uâá?÷rÉìG¼W@?7àÁ÷?ïÀ"¿óuƒ?ë§xª`¼¿åÄíz¹¿äM5<ø®Ó¿ê'`eŒ¿à_ô¯iåOTHERunk7C 2252+5740?ÔéJªø?À÷P)Ê:?¸þŽÛ$v?È󜭨ÍÈ?âk‰<‹õ?Ņ"â9_a?à0Ö	—c?ÎW i±8?Ñ~¤!'?‡ÉbEU°È?Þ¯Ë鼶n?Ã`D¤0?å:Q†Ê"è?±ÕäÌ> ?ž`6E€K?GbŽAV?Ó¥\¾Ðhk?°ø*ó+'Ñ?æ÷ØÆ*F?š[*MOvÝ?©ƒw|åä?€¹`-š?ÍÀê¿.²#?˜,X3ÙÝh?Ã/ÍÅI?¸'åÏ·"«?˘'rê¿?Ñ(·t 
g?äN	¸2~?Ιo»'U8?ÌZƒaÒ`"?½{é/ƒü#?'ʾ`ÀŽ?•Ì=™?èS	4\(?½ã¶7"ðµ?×â]±û©ô?´Dt€å?¨ç§\rÛ?•-óä)?â€V±+uh?´‹í¸Äp÷?Ý{Þ/<)?¥7ý¾	u?¶Ž}—£?•q¼²á/?Üà'pL.?£üjšÇ}MIXED4FGL J2258.6+5847c¿×.¥4"—¿îSíPÑÀ:<§Û{¼9À;ŒV=#vþ@ E)ØÁw¯@j[{PÙ6?ÔxžaÕ]?Æ0C>Ä?ñ¾Â³nVö?ñev&wä?Ä8AåӃö?äÅhT}0¿æµAjÙh¿ÜýI׺f™¿ëqáÄ«–¿Å!]Þ,›"OTHERsfrSh 2-1520?Ó~ˆàӄ?ÀlZØNò?'½<9€Ð?ŽSëތ?åçVÙßž?Àw4%1Îë?іÓóÿãó?ŒÚٔ?¢´ðÛFx? 	¬4Ó{¦?æ	FøYdî?Å+ƒ"Œõ¥?àxË#2Ô?²ÍmX3x?¥3rž-'+?–}Ñæ1æ?ÜgûeÖ7s?²d~](?Øþ!ñ
ì?¢·Ñ˜,"Û?»¼¡S"x?—ùÿ"h?à	ZçN¥¢?¢Ç%'0ªÈ?ÂgøÂt]?´>ùŠcÿU?¤^-ƒ'N?¢£àáªõú?ê öæ%ä?¸ŸSõxý?¹vҕ‡½Ù?µÕP±3ÄG?¤;ÄgÈ?®¼®|­Á?돑ûÀ€8?¹%Å¡Ï?ÑhìJ
Ï?±7¨3¡~Q?²_7þŒ›?Ÿß§ †n?äÿ¢ö˵?±%pSAsý?ÅVLpy˜? ™QÉl?¿."òô\?¨I…L^?æÕ©ºÎón?ª·¥†'pMIXED4FGL J2301.9+5855e¿çY§bœ¿ðy`>.9À8¥ÞC¯'À;jÄ$"õ@ "öøogí?ÿµè"¹7Å?¬AÒ³@´¦?«"͏@'2úÿ?@WÚœ&¿ÔEìþñb-?êÓÌ@
>¿ÞU…2à'¿átA ´@¿ã3>)[n¿ÜÔ¢¯OTHERSNR3FGL J2301.2+5853CTB 109?è¹R•ŠQŽ?´Ä•4Ö?uæ~¿m§š?f:"¿`x?Ìk²‹ò¬?´<=°Ö?Ò~ÝVÃí;?ÇOUTè‡
?¦´¶\q;?¦Ë|´"CZ?å^Ö	a}ž?ÇvV&/ó?åïX̔n?´¤ÔâÐ?˜j áÒç?'5ùñyþ"?Қ£œt6Ö?³
`2Få?ä­Ip¦(?¥âsA?»%H¹Ø(v?–J©c¿°?ϸ5à{o&?¡Çêeí?àÝúà9Ù?ÁUtò;?'Ñ<řæ?"Ò§Z·"?Ýös†¬Ï?Á.'a2 ?·¶gR?À7'åxÈÇ?§öY^Ò.?®Vft=Å?éҬЃ¿?Á³xŠLÂ?Þ T
ÉAR?¶ÂjŽk?œ<ZX£öŽ?îõ¬ð?ߛæLÇü%?¶D½±ªF5?ÚØyŠÔ9?®ÝÂîp™B?Ç*9†ÖÀ¹?§G"RNp??ْi±kê¬?®%ÊÑá8ÞMIXED4FGL J2315.9+5955c¿Òüáøƒ		¿èOQ‹N}À9V®ÃÍIÊÀ:öÕsd{«@b‡üŽ1@jî+¸ë?ÇΊ<."x?ÇõíÂæ™ý@˜ÿàöO}?øÀÛ­:`N?ïÿÝe¡D‰¿æØO·Î8¿ä»P£‡¿é2*õw¿êìóžGÔ*¿ÞŸ‡ÜôOTHERunk1RXS J231543.9+595510)?à$áƒ4 ?ËÔ	
–?ŽiÝê+'e?†¿xÓÝ%?ÞÚgMÊN?ˑI°hF?Ђ†:ŸÁ¯?Á™%Þêd@?©%h=Š	?¢ãŠ~s£f?æ,fbµØ?Àö@ƒÓ´ž?ÛàÎfÕÌü?´"ŠûŠê?°òŠ'{ÔH?š½7ƒyòŠ?ßâŽõ®R?´0?–Žœ?Ë%Ki
?šK%½
?¿:»äXjá?'_fËn±?åS_1$ '?œäìžPˆ?ÊL÷Zü:?ÃÏb9—6¤?'d~£¬¿}?K­É"8?èٞ4V?ÄFvf¹p?´zф ô]?­h&4;(È?«]ÚÐÁZ?©ø>HBÂ{?ëºÈ"™#?²ÌÀ5Sø?ε
ü ' ?°Ý/ßU`f?³‡õî`‹?œJV=ãá?åá½Ã"1·?±óƒSö»ø?°
P<¸ªò?Œ("]øٛ?È
À‡ïù?ŸÿBíoÂv?鲈}èc? ,N£¸<®MIXED4FGL J2323.4+5849?Ë>ªŽùyÀéÛÑLŽÀ7'BÁE°
À:úïY­@ۅä°ï!?ýîy	×W?šKc™å?²³	¾U÷¿@5¿jäz?ø:Șµ˜ÿ?êVð§h[?ІÁOÁs¿Ø€Jþ€ùæ¿ÞýD
öä¿ãÒRþT¯/¿Û‰°b³ÔXOTHERsnr3FGL J2323.4+5849Cas A?Óͼùgç?ÆüšoØU?«§BœÚ,6?§=ÎXb*?ä^­YŒZ¹?Æ¥çõa?¿X¥ÍHa‡?ÂOð»
úÒ?ÜHXÀʝ?Ìa 촞®?Ûá}̒?Çaݜ$A?ØqÜüšÅ¿?µt*E	/»?¸¶'{NgÞ?¤ÙDOçÃ?à°L';µ?´¿PÓP¹?´'˜?ºŽÁ*UŠ?ܼ³©T'?³ƒÁ¼?ÙéHM.?²å³i¥Ý?Ëf­[öÔf?½2š–i?¦†üÓpm?ÛVIÛÎ?ç½ô™^O0?¿4¼4Ϧ?ª¥"Oí?·EŸ†Š?ÞÊáæ'??ÐmájÃQ?Ýàk°RBÃ?Í~äÒs?Ó[˜dÝ?³-‹³ýÉ?³ËN±¡Ÿ¹?¢ûèQ¸?ãØÉ÷Ÿ"3?µ)öç µ?²±R0Åê?šk®Ö•ï?Þ_ÂÏ.71?»ñ«ÔY³û?Üóè¤2"•?»}ÐÃÚéNMIXED4FGL J2326.5+6122?ï£	F¤f?Ì9Ê&)_À:â¢÷ç-À;Q·ê½xœ@›, šTU@3«ÉGO?Ɍ'sZj°?¤~=šZ?à91yõd?ÿÄ¡ÿ?í¾áÝU03¿áÚñR¾¿ê7A_ƺ¿ßÍbßHOz¿êÅV¶Jª¿Ù±Þ´Ö·OTHERsppSNR G113.0+00.2?äkyùɸ¤?–͒֘?…< îmH'?|ûMÒ:†Ï?Ö'03?Âz"±šŽ®?ÕÉ\NEÄ?ʋ:9£î?'¢¹±o¬¿?–9PÞ³·Ï?ä†^"M_¸?ÉããæUJ?âoE)¢?±K4º½mÄ?Ÿ&ñT˜=?]xÕ36?ØíhG¥Ë?±Y»"NN…?åïÃMX^¢?¤'³]–ÝG?—ºy숲t?véçÓ	£?Ò¤ÑƆ·•?£ïv–›s ?×)…I&K?Âr±Áa<d?•ÞV8Ñ?Òa{z]?ãÂVŠ·dÂ?ÂÊ7q0nÞ?ȝaý\?Â'ˆ
ñº?2³6Á&?š½"Þds?éxÃ"ð?Âb6Mf\£?Ó÷™¯'Ô?±XƒïB?¦Êow¸"?"bûÿ""4?䗐Áiþ]?±…G!- m?ØÝ¡<6xH?®"cÕ¶'?¦NÛF—{ù?3wÈ>?â,A­Û,?­â›fßnKMIXED4FGL J2333.1-5527¿ëAÿÛ©ÀM)f@¦¹=À:I-(W7À<Žï¼»Ý'@í¬АÒ?ý»í·(Ú?Âz‹÷Åsè?Ô°"‡áá1@ÄÖÓõ¶?ø9‹¼â¿ÒÜ"'Z¿É§<µ¿Ü\2/ýô¿ãv=öÔ¿ë‡'aBæ¿ïý|Í°ø[OTHERbin3FGL J2333.0-55251FGL J2333.0-5535?ãVoäP?ƒqï±~=?Ð(¦Y©·?¤šÔ'?ÂV>Q?±ï¸4'Ã?äl=Æ3?ÐSHkB‡ÿ?ЩÖï¹{?ʗ¡åËÿÑ?¹ó½£e‡?º['¥s0h?Úb4??´Éðsœº?ÛÁsIÆ?´»eé‹A?ÄüùaUZ?ªý‡•50ä?è•Už†Ø? Gð&뒐?ºüÕ©?—æíáú™T?À¡Z‰ŸŒ´?—2?Æ©?ØîAÒt>?À–çFºh`?Ø&h/z?ÃöªÙTg?Í×A‹Ì¸'?¼M£ªr7‰?àä8"J?Ѩ}E3?صŽö0&?Ð.ƒE£½?¿zڀ?»-S9&×?Ï.À&÷?´^£5¹E?âcrÚ>û?·"<V?ÇC¨ p
?­ÝÛÂýÎÊ?â§éûµA?°TyDރ?ÄnàÞQ¯u?«˜;Mš?Ðx»™"Ý?©rÍÇþÅMIXED4FGL J2357.8+6231¿ëÄ;¿ÚÝ?Ó8ªŠÀ9IëoOCÀ;0Úb·…=@qC~Yø@èÞæªÄd?Â1›X‹‡?ƾ	e"i1@QBè²Ü?÷a,Ór®H?ïÐøuÈ9¿ât1€*²±¿éÚ]C§õ}¿ç…öº «¿ïÿ4=ŸGÙ¿ïåﳁ¢OTHERsppSNR G116.9+00.2?êí¨—á3?º­æòV¹? äO¼Ë}?°2ÿìÜ?ÀIÞ4B?´N;ׄ|J?Ã9·NéМ?ÁŠˆ9tëº?Ã5òÑÕ[x?»·-ܺ´$?ædwÐ4û?Ãû±YÝI¥?äÁ"š½9?°3AdP?³ÁÍ©y]$?ž`(ä2—?эjP·¦?­Nb»®d?ËüL;±¡?2¾hQ3?Òô>°Öc?¤€àŽ¼?ß
µ©ßPÍ?¤K!‡j?áÖü	À?ÄùäZæ‰?¾«/Ý×ü?µ`#Ö?ÔÊ ˆqå?"Jª³c?­ëæ¹*o?±E[Y?Ã^+Sç¢?Àu©5ª&?éI¶Í‡ð?Áܽtƒú:?Û³ßúë²Û?²ÿ$|¥Ü¸?¾Öí7%†!?¤ô21"»?ܖd¸]Ì[?²òß¡‰Ôµ?°éÊ×8½_?ŽѦ¹-W?ÙVè$þ"k?±
ïÁiMi?á7R'§•Ž?°Xˆg¤VMIXED4FGL J0000.3-7355?ïåFýP´ÀE]a€M˜9À;%¦Ñ€ìÀ<ʞœ7ً@ÇÍz3£@f»üÊ?Çõ€ #v}¿®0C(É£?Û
ma'Pþ@ #¾ööA¿ïîa«ì?ìª'á›eø¿ãJ<߯R"¿àÖöâv¿ãڏÎ>¼Ô¿ïûSÞNjUNASNone?ïܓf4[?pÐ6Ŭ˜?7˜×rPvQ?4$ûK*?p<¿p
D9?p5OĺÐ?ïã½F>u?m'ýN7¯?3—¿øDŸ?A>tXˆ?j‰J…@?jA¯9Ieå?ïXÎÈPU?†p]üƒ h?b#ÅÖ\¬?dxÔ"?'¡ÆíBk¾?…BJÃÁ·û?ïÚH)Å(?SxXi¶ÿ?Owb1­]?3Ù:c¿D?mðøÑd˜z?Rò2g$_,?ïÅðWü8?v¤)8Rµ?Gò©‹?Aúß/Åk?z	®àÁ¶ð?uÿXe?#Éß?†T»ÖöÀh?G_.9Õ]ó?\ќ®a©?†EiWÉp?…
³]+?îô¨Uôÿ?ŒQ"†à"x?m gzHכ?p%Lú˜Ú?¶èXR¥?Š`Û·÷'¿?ï wBÆgó?pž,QrÞw?aXc»³—>?QƒAÒN—?ƒŒo÷=r?p9à‰ YAGN4FGL J0000.5+0743?ېÇÞ{uíÀJƒÅ?9ѳÀ:πhp+âÀ<t3⅛¶@»?ö;\?ýl½³TUÃ?Ø·G?Ëç?Þå¥vF®:@JFsBî@ÿ_Y¬Å?ï¦'ÊÖ(¿­O·½	úï¿à)HÎ¥êá¿æ™¸:lã¿ïÿãzŽ;˜?Ù­ µTUNASNone?ïu^¬ÄÖ?eØ-mÔ?W7(`ž\Á?W)Ë3"Iß?Ó??ÐEM1m?ïˆPPFá³?†q!-áµs?hj…ŸY©—?pén—š«?‡ÑJyºšà?€Œ­ùÔ?î˜?v"ã÷?"-Ɛ1`×?Œee§¨Í?‡ŽçüãqÓ?žÅ^Røsº?VáîZÌ?ï *Œú?x{˜ÅÅÄ?mBZ3ÐV?Uu+xnC²?˜U/_Ó ?w>íkØà?îØ8ovõ?¢9¶@¯?nž‡ã¹KY?mŒŒãGt? 'ŽH¦º? »?'O}«?îßÈ' «F? o<Ù;Ç?xÁó`MˆJ?ŠBÔåÚ<?Ö~Ec#?™¹ö¸+ö–?íºPÚý«×?÷Ù½az?" ‹3äÚ?‹ÕzEko?ªŠã
%?˜á(tIp:?î*"…W»?'"œ;v?rãU~zlø?hªÕ%Ó³?­ íM8?'¬äÓhmAGN4FGL J0003.3+2511¿êÞ¨GîgbÀB4«ùiäÀ:¸üþÿÞÀ<|ÆÖƬ@šº²˜îú@v€$}Ê?Ð>.ϏÐ?Ԕ6ê'@\¯-•?ïÓێ¨ò?ïƹT繿à£h_Ýƒ¿à¿½‹ç)¿çk½¾<¿ïö({ILz¿ïÉÏ÷úxUNASNone?î¯#³RA?©Y;üø'?ð՘]ç_?Žnæ3ê?«xØa‰'?§!T	RË:?è™Ép)'Q?È/ÐóM0?ÁVëõ&á?Á¿J–"ÄÔ?¸ƒÜ•ñ1?´Å}aÐa?챨‰v‹Í?¢7[bX^? ">ã"v?'"ºêC£?²rª'´NÜ? ãW+I«?ãe 嗍À?¨'j&†Ê?Æì0šQ¥?£6ªºgë-?Ën9w\?¡kIÈG˜J?ì;:¬?¯"ÇN†ì[?–ÂßâH÷û?"VŽ˜cØz?¸v^11Òë?¬%ÂØÉ?âJÑa©_­?Ïê9vöN?ÎO:‰Øu;?ʓôÁ)øÄ?ȅñ§Í?À´¨qVb?ëW'#©Rt?¦R4Š‰ õ?§$S
Wá'?–ߦ¹Õ³­?¹±M]‰{?¢fÿUUm?Ö·Ç-6Ö?®¬P€?Ïâø›Gi?²Ì[¸JzF?ÙV¼…:?±øܒÙ?MIXED4FGL J0003.6+3059¿ßêf-4À>Å¡fµNÀ:ô™aeu¦À<ê)\ðœ@fçŒí?ýK˕•(?Ìu9èÙó§?èŸüàõ–@é™Á݅'?ý})vpö¿ê!—à¿ßAJ¸Šöi¿¨€Ua¬{¿èïÎY"ǿ隢ãÅ6Ö¿ðUNASNone3FGL J0003.4+3100?á¬áÈSä?ǤLÌÉ?ÖRŽ$<í"?ÅΔ`}Kä?¹U€_ܗ?­iz<éÃ?âùL]?Ì¥B*ƒ'?ÓÖœ¾Æ?ÉFåøAð?ÀJfá5"?³€÷ŽcÒÛ?à\ô'{­?µp§vÀÀ?؉½]îó"?´4Sm)?½~"è×G?¥B¸Ã|:?åÄõJodè?©¯JƐ?Ç×Î	#s?¥…ç#ÿÓN?Á\»9Hî?œüD²A?ÛÝ`]ã¶?Ãøp'lÝ,?ÛÑR_•´)?ÄöX÷½ç,?À£"'>'¿?±ð2ð½ª?ÖºÖ³´?Ì;$ˆp ?ÝbcXP4\?Î	–›|7?Éáø/I?½•Ï›ÅT?Ö4é;mie?µ'TÛÊM?à綌æÐ&?¶É5¢">?¿î¦«Ù@?¦ËÏ´¤0"?ÚV …AÚ?´4­Ü.°?Ô5wƒø¦"?µ&+'<ú?Ñsø['?°4b®9½MIXED4FGL J0004.0+5715¿î°OÎ}Àj<´¼5À:
ö¯õ%±À;øãȑԩ@²á±
y@éÜÂä¿?Ée¶h1m?˽®·8@œC²Ý7~@Äó  ¿»ž#þ8?ï3À¶‰?¿æm4§§y¿â½˜çÂòX¿êÄò]€
׿ïý."hqUNASNone3FGL J0003.5+5721?æÊór—»ã?º98l_¿?Ÿ>Ä#ˆ÷?'$DRÌGð?Ðv,×úRl?¸~šB'?倲EÉ(?…3•¡?ŽøåÅÇ=ú?ŽóÏA²'?ÔÔF$á?ÁóÐ9òG¹?ê,'£v×?©¤{';ì?¤"Ý©3®?"ô0¯nnÓ?Â*¦«¿¥·?¥jöhœ?뜇±J÷[?'
@-"#?§"®ë"U·?'èͧE?·YjÿæJ?Šâ»œYڕ?ÙÖ²ró+u?À›(ì?²ŽRIÁ?¤¥)_B¸?àÒ4 ¤-?¿ìɨ'?i?ÙNTEk]á?Æ2ªHé?K
çÐä?¢Oå2®¯Õ?âp"…MØ?Æ7qÓ¤NÌ?âLÙTšŒ?³p6&‹7µ?¹'‰Š?£†=†ß
?Õ"-q¨8ï?°ª nRa?çg¼ö‰?£8ïöøŽ?¶bð›K/?—]Oïßÿã?ȸè¿F§Y?žãš!\y±MIXED4FGL J0004.4-4001¿åU:$q¬ôÀRvñ€
À:¤ˀœsÀ<¤@è'œ&@M®$ëò­@Ò=ÕM¤Ï?Á(òg'Ñ?´Q
u#î?ñ
	n=Ë@\nóӡӿ؍«dGRO¿â
M++ýµ¿ßdb–£¿ÞÇCuö|¿éw±b
;R¿¨ˆ¤B®ÀUNASNone?ïïóyE!ƒ?œ¥.v€§ë?RͱÝ0êÓ?œª|ípÄ)?J–·]lá?:J¦žèº?ïçeDRj[?i­D÷IÛ¾?2
{‹ëöÔ?>סčÇ?fYlaãÙÞ?g&ôÕº:.?ïÄþ.ϐ?i®È_˜(?SÜC-n?Z¾á{ªK;?xº±—<G.?dêÄ©ò"?ïàÍäé'ð?L…¤%!7?3ÉÊ(ù?¶s†R5Ä?l¸áçõÊØ?KÜøi'û–?ïí߯±·?Q¶ŸtÔ?D_h$gw?7¬â
ì¤C?Zìˆë%Ç?Kâ€n?½ï?ï´ºîd2k?"ÒVE?E m³3¶ø?Vs¶=æ«Ë?w=_í?'¾¯áV2?ï ërá?t"~]\{?^&ADÝAr?cþ'éµ)?"Så•ÓŠ?pˏO†­†?_Ñw?m"–{|*"?K5P š?:Œ¶Î¡e;?…`îêpX?lÛç©;]AGN4FGL J0005.6+6746c?æí>¹=È@ åæyF=À9»g
USÀ;8Ś©d@«sP¯šã@Üï$©Á?ÎÿöZdÐd?Ï}Æ_@ð?Û¸"@ó…PalW¿ãŸ£i&4G?îÏ`%Æ¿ç
.Ýc¿èéRáP¿ëžÙßÚƋ¿ïÿ/?ޒGUNASNone8?æ[–ƒ‡?½5Cٞ—?›ÉՂ›(Ï?]#õèï?эK{93?»ã´´–äÍ?à"dš¹Í?ÄWŽš• ™?µÛŸáLÚ¦?°þ†õ6?ÙbNåÒh~?Áï X…¨?ãí?š/ý°?±Aƒ6 ~?°à÷à£x¨?šöå»O¬?ÓíBÒÒ97?°ÔÐk+·?ãP6̊?¢B= Ì7?·¢«IÆý¾?'{tæbÆ?ÓÜ´ûŽšý? sÐ@º?Ñл?—Ö²?½2=Ęæ?³:Òc傦?¨F9xÜ?ä°H·dR?¿4xÔå(?ÐÅk>½U?ÂÈ]–"¦?Ä·[gkl?ÀDþæk–?âos†=$?ÅWĵڠ~?Ô8ØöÉ?±x1	ÐH?½ú+Æ,¨?¤YþĀH?â$Nâ®ê?³u5uÐ?ÕªIàHՇ?¨_PÝ
Þ?˜ïm¿(Ó?¤¯º2å\E?à"Ÿ3âZ©?ª…Ó\*MIXED4FGL J0006.6+4618¿ÏñVf`~'À/½KÏknÀ;;·"¤%À<"g©\…<@ u™Y,í?ù,?£ƒþ?ÝQcŸâˆ÷?âi9Ÿ³äô@$ë7ò@?ù\ͶW¿ˆf_Ÿ;³Ï¿ïùš@¬ó?ímÿ"Z¿ÑÈýú1¿â%¢@Ýî¿ïÿñhUNASNone3FGL J0006.6+4618?ïÆÒTÿ"S?lÀÿ©3æš?WoÓ8S	?N"QO…Ú?vºàÀq¶?ivdÅ®HÉ?ïk®i+ßú?"Cë<NÛ?m5ð>LZ?uÊ͙Õll?Æ驔rð?¦Ó0A¦?îՓA(P?'y>i?sÓ΂ß4Û?tD¼‰'ñP? ,U®¿7ç?'¨²Ô7¬?ì÷"u½hÎ?"1½‹hä?s·"Ûõ?`EHxX›?· ßÿœ'?"PÄ}BØ?ïqqüL¨?†åøº2ä?qq^‡E?k­å¨Ô0­?Šë/··M?ƒ®:ük?înC®g?«XŸ&ÁøÃ?'Ç
S¯™?"v)x¨?¤m³—­®?§W•‡}?íë]/ŸÄ›? +j6á…Å?yWdðŒpï?zнÁBà7?®@eŠn:?žÕØÓÚ÷Í?ékŽ]??«ã•±´?uEìD '°?q¦Íìªá1?ÉQ¾ï>'¶?«ÝYi¬*¼AGN4FGL J0008.4+6926?ï#¿ÝG°@Šü‹y£À:S\лnÖÀ;¾=‰ÎJ{@ Á<JÞö@ïþøþ"?Ê	¢Ö"0§?¸—=í§?ñi!—)|Ñ@¤5ÂÆ¿íÓbÙð!?ïþÚ0bž[¿å@£(Ž"ƒ¿åôûTŸ"…¿ÚW3£E"à¿ïÍbUNASNone?è€s:è¼Ë?½éÀÒ²XÇ?}ÈŽÑØ?'9ѶU6õ?Í$Ҕ¯F?½†í[¶?éI¡~aÒ$?ï%§¯[ù?{3Ø[r)?ƒY¥Fû¯?Éÿá×ËÙ]?Ã04IÍmJ?ép*½÷P?¬&#‰ªµ·?šý_ÝM]?'z=QÒØ?Ȗ"Y'}a?©ÊÔ%q?ìË&í³)ì?ŽGP'Yº?""½'Æf?jñ­|‡¯?·0ß¿ðP?³·åÐwÿ?ã>€^4=Ê?Â.6:4ëU?'æØ…N?˜ölñZ?ØT—%9å?ÂÜkP[?âvªÛz(?Ê2c·Væ8?ŒÏeç)‰?–™CZ9S?Ú,/AA5?Ɋ)Ÿ$?á»Êcƒ¤?´£ág=ÅÁ?©BnæAÜÒ?™éŸ¬³EË?Ù`\1Y>?³ž§`nº$?èQ

è2Ñ?¥Œ"ƒ¢XÒ?–Fb
">?†g3¥OÙ}?Ëó'|¼6?¥`¼ù%mAGN4FGL J0008.9+2509¿â^…›N¿EÀB\¿]xÀ:§e
EÔ À<K>I窟@îÒ09@" 5•
?ÏÎç"3*û?Èntý­ë5?ôÔb³S@â±³kÒ·?ïBO/èû׿Þf7l}ל¿êDP\8åû¿í}‡Ÿœ¿ïþž5àŒ¿ï€ú)&jUNASNone?ïˆcE—b?¦u,\ÂÜ?a*¶€Ï=?d+ŽçÍxÖ?‰œ€ð#•¼?¦RtGÍ{?ïBÏòµÙZ?'†BÁôì!?uCNøKVÇ?{òÅ
ß͞?'U-ð-n?‹ûJ=Ú¹Ç?ï	äz	þ©?‹0H?vŸ©Rp!"?u…Ã0?™†b=Š?ˆqŒ½Æ¨#?ïtl0w?sÒ¸Àžn?l$µsï?`ò×kæ?"¶yÃH&?o͒«¤ð ?ï\(©†:†?—r[6øß?oȍ~×?m¾EX£Qù?šÇâ[?–Œ©}.­Q?íãÙĵ"º?«TƒXó2Ó?‹öNk?—èˆÌ	0ë?«&5gΘ?¤;Xkˆ˜?îa¢åÑ3?˜×ï™3u?‰xy,ty»?"»Ûy=!¬?¨»Ç':Kc?–îu-F?ízÍ£âGÞ?'<ôìÀKú?"×·^ƒ?ËìüçÍ|?®gJf³W?üxB#>ˆAGN4FGL J0009.1-5012?ßýÓÎQdÕÀPbç-¡"ûÀ:kõ²Ÿ$À<'ò®2®@ K¤ï
?@éÇ´_?ºÃˆ€l¡ê¿¿:_nÇÖ?҂ú;h@	S6Þ¹^?ïÿlýY\"¿×ö%ö4¿è>O ¿äöTðóÿêY*ÿ1£¿ïÿ"¯ý‰-UNASNone?ïô†¯SŒ'?QQ/˜'?-T–!u;?'ž² /?SH'Þ/ê?NÅõ?à¹Ò?ïêVx»0K?i/мbå?2,píï?Cdœ^Öj?ccùy©W?fÄ¥köÒ?ï…ç#ÌI?…Š¥Ã›9?gpM|«éP?s™ŸI?ˆÞòá€ÛT?'§¾a+ig?ïêßkàÏ?CçšÃo"?D€ûWxç?+¨)-Ú[?`Ðá­ý"Y?A9¦½þq?ïæø1!¥?ba"*~µ?>ç\:R?7Ï{?°c?e*ã3»¡0?`íÒ}Í?ï¼ñè»é?ƒ{!9Á¸?EûWö?Xƒå¹?~å,*…ƒ›?µŠæÎU¹?ï\`"€^?‡ö‹v¼?m;Ʌ˫—?u~êpëˆK?Ì"Å¥zÉ?…ù…i?ïÄùeïQ?b›Ôëªâ…?^«34¶Ç?K»ޜy?vUk'?_‰
BNAGN4FGL J0009.2+6847?îÕðЕ·À@ðù£v'À9»œ`ô6žÀ;f?Èc@ïÓ^y@Zh+b"?É$•vjN?àÕJœ@iž»'?þ,­.vá¿Ý.Íb¿ß%"?]ä¿æ¬\꼡ܿì¥×€D¿ïÿ'`4P¿ïöU\Rç.UNASNone3FGL J0008.5+6853?Ô]F,ß? T^Q"?Èpt<XT?¼"æ'Ää?ßj´·µÁ÷?ÅíÅ3<?bØMš¤?À£­íl26?Þ$dQúÇ?Çjµk^>?،êBÃ7ç?ÄT¦.—0ø?ۉžë¤9—?´'°Z?Ê^ßL¬+?¯zKø0e¿?×G\¥ÈQ?²¯ß¡eÀÏ?Á_˜v®Ýù?˜Ýçñ4n?ߢ6£–¯?®´V^[€?×­ý¯Û?¬Û"•òÈ?¿.ýë¢?²Kݘ?ËÁ^h¯Û"?¾G/`ã)?å)ȨrFç? öZ9ÝF?©ã%ଁ?²¾ÉÀs†?âÚò»…?Ë uo²";?ש]`•?ɬ­£øÔN?Ñó¸å!?°¤L\"MH?Ð/ šGr
?µ˜ØUKsâ?ÝܦÕÓlà?¶žo·s?ýr3aÁ?8jÞzß?ã8qR a?µZ‹$>N?ׯF9JNƒ?´ÆÇ&gYMIXED4FGL J0009.2+1745¿à#Þßý_ÀEû‰a=1ºÀ:ÊZõ1À<ulC9@õ'ßÃ@fàÄÑUÉ?Ӊ7³Ët?Öüàü.º(@±FC±/¸@uQÄ?æPËßçܞ¿æ~ُRá€PB¿×¿ëb¤À>I¿ïý¯ùWoS¿ì0>·çUNASNone?ï@-vÓ"?ˆÕŸՂ	?f-$U'?ZªZ5óX?•4°>JA?‡jPhÑñ?îìnÑ*;?›ÑœBÕãX?2Õ÷åŸ?ƒyz¬LÜ?™æg)d:X?"Ý;	4iç?î·§ÁFÿ?'ÈÑ^©í?‡_£ÍÏ?€Œ'…3G3?[6¨Ò†?Œ"
…ÆöA?íü2RZ]?'òßgÐe?‰ÂQ¨üÿi?jô¥ò)?©ÌFr³¯M?€]Uࣤ?îdv­A¨?›CEH5X9?u"³Š^n?l%[vδs?§â&%Xª?š:T¿¾Õ?í
úÍQh?²rl|Q Œ?"$¾ÊW[ï?¡ò %aÕ?²†ÿi%_??¬×ïæci?í?֛=ï¶?¢SZ](+?–ªf–C,?ŒŸøu ¸?°V±5â‡?öûIŒæÙ?ë
|ô,?žg™ª&'ß?–+¬¿Õj?"_ÂÈèíº?Á™ø††d?œ9I­"AGN4FGL J0009.7-1418¿Ü
ò®~ÀRz^³¾#À:y?Æ¿l'À<Žè´‰ßè@"êžnëp@{èäZˆ?¾ñ[¢h?¾}¹"6?ù[åô»ÿ@1är…Ùs?ïþð çkµ¿Õ÷Å^nuT¿éç`+¹Â.¿énlŒñ¿ÖÄ¿ðUNASNone3FGL J0010.5-1425?ï§XóGq?û	…??Q·;5Î'?O)»hljd?ƒòÛÈâ
?€9J֓L/?ï½{Œ¤yÙ?~"´Ð%?U
š{û|?_-7_‰œ?{âvIãÄÐ?xËC—Ò¢?îõG†ÒB?ŒúÛzzõ‰?rÓÂA{óÞ?r3P×-?œ©¦'
[Ï?Š¶ï[f.è?殺 ¯§<?aÎj¾@/?_<X£íŸ?HÅcäk*Ì?xC'S\?_(W3®ÞC?ï$ô7—=?"LÒ,lX?l¼ÜnÕo?p-Çûß?—çeï®?'ô|".?ïNžÆK µ?—=°¬ßY?htUFëL?wˆM×É?"œ•nÞý?"	¶[ê\?íø;Ù}'Û?™+ìÈІ?ƒ¬¬-‰gÖ?€ž˜væX?«'Y¬ÒX?–íxöþþ?îù…h?'"W|az?xêãdDl?k¤}s)_£?š£6€Ž"~?^[¾AGN4FGL J0010.2-2431¿æl½Óa«ÀTô±î$5À;}íÎ¥!À<àINþjÕ@CÇDø'ˆ?þf ³iNx?×kWÅ®K?Å2äƒÍªm?텯¢šÜ@€­ê´iT?ïÌGkÏ[ó¿ç`.ßœ/¿åÎ=_Üßj¿¿ô/7w)¿è
˜à66¿ïÿ'¢."'UNASNone?ïæ#¯ÿÙâ?Wn
O‡ML?:'üñh¿Ö?+"pnXGr?fŠ(…ôæ?U®Œ8.±?ïÃxšùõ?{ÿQX€&?R7Ó\…%g?ZØBTkð?yæÎçhV?w@Ýz¡‰?ïq1²™^¥?z¡ÊYÆÀý?b¡¥ß|— ?]Uóöá	!?)ä0êÏ?xñ ¾"a_?ï}4ç›ã©?n+€÷3@0?QÂö#ü?<øG8{^ß?Žz"‰Í9?me¿í¬C}?ïÏ]úª?l—Û1t+H?JGŒ~ǵ?@¸2Xßa¿?uG'T÷·?jH7ñ4?ïuCšÎ;Ò?Ë` …šT?]¥n©z¾?k•ˆÑÁò]?Žúi=DY?Ž,TY¹þÁ?ï€ Tfè?…Ãædǁ"?l%Ö}r=?f{_àxð¿?š+A9j¶«?"Êvdâ?î˜^Ð3ÎR?‹¡OnÈ͞?`Z0ªB5f?VtxÞE=Ÿ?¥toî™^?‹}?¿à4œAGN4FGL J0017.1-4605?ïô$|áýáÀQw_™Ã‹À:×íø–3À<©å
5r©@¼‰:Ѹ@*╶¶?Ã&LšãEµ?")ÛÔÁR?νÚÁ'ï?þ¿VGµK?ïäE#öN¿ê˜Ô½‡	Ÿ¿è–­Í-E¿ç]W>UP?¿ïþ‹ Z›¿çºñ£EêÆUNASNone?ïæDÓÁB?hÄ.ÙL?V¬Oš˜*W?Z@D]ýš?\Ê
xK?`Ôeäà¶?ï«·ÛÆ\=?'ò¦|ޖ?`Ÿí.E?g?|›å¶?€íáCÎF?~	øzCHÅ?ï{5LàP?Œ}
ëÒ«Ç?/M	j,?"Spw"Äg?"Ù³þÈé?'´êÓRï?ï£S®¬?e棓
¨?q´t"=ê*?XÂ=Ûï?|¡ÿÇÊ?]z:˜ªÝ?ïÜz¤áÌ8?mhDMe?bHgŽ¾L?g "\¬
ƒ?a=AËB±E?^–0Ü~_?°eŸ? ±‰`¢"?tê/,˜?…¦BLë;?˜Sœb¶Sp?™
ÐÊz?îˆjáäû²?"Γ¡]m?‰~_ù²+?‹
:ôü}?¡62Ki¦[??7HL½?îîVû?"ÙÙ<×'Ã?‹:þÊ?z?|¶?²¿?"žÕÑTÝ,?|·éóŸAGN4FGL J0022.0-5921¿ÚAê‹y›LÀL°Èÿ¸²dÀ:sÕzñ7æÀ<XCëè@Ðu¡æv@…qŽ¸•?ÀŽzV³@	? !ÆyK›?áuÒ"4Ö@Wj^B«v?ïý)‹ê"n¿éb"¿H¿åVŒ¿ª¿åF^ˆ¦¿åDmþ5O˜¿ïýÒÞߞâUNASNone?ïÆÆÜP€ÿ? -k''?JaäU-š?l<4û"–?yPUiÔ.?œì¢!,¿?ïÇkð+Õ?vòáC\q?MG¸«N?Q…jÜ­l?x¡'ì5ø$?tÄQñìÄ?ïl/ÿ°?~ÞÖÃ#^]?a]誂,?Qâ©ËÈmP?YtRœ¶Ù?};Xẏô?ïy®ª†ô?iͅØê5í?aQ槔Y?Bb=†µ®5??å𠖭?i(r8LdÂ?ïnµ¡W»?‰ÙÊ6DŠž?_÷¥9r(ó?[ƙӸeÃ?)уÂw?ˆ'¿§í'¶?ïoxÓrФ?'4aFñõß?Zÿ^dxFV?e er?ùm?`ï²iš?}©fc?î´Rdü®è?''HM"à?p‡Ç½ùà(?fÀ"óµ?¢©à´lK?'zU7"4é?î^õ{™?ˆÞú©N?{e!'/¿f?djX+ĸ¯?¦¤ʍ ?ˆséÆ[-AGN4FGL J0023.6-4209?ÄÐÈq•»áÀR{½øôsÀ;kÿñÀ<ޟ›;ZI@â#P<@Ž­\Äüõ?ŕá"!¿ž¾¤k?Ú*Ÿü4C@ü‡ìóß?ìÁ?ûÅ¿êsÕº²¿ÌüòCÿ´+¿ã±L]üŠ€¿ïÿ Âg%?ïý<Á§TÃUNASNone?ïÞÐ%ØèË?sûöï'Æ?Q/Šbi3¥?_}{€$æ?h˜+|'Í?mÝÎ×ÝÚ¹?ï͍6´Çó?yld+G‡K?K<…ñü?UB$á³O?uÑÓîéP?uÞfm|?îýJ^'?"]|li"?€"+°á?"í	2*?˜K¯3'\A?Ê}ž-«?ïÑÃË,Ÿ×?\óP³æe¿?7ñ&¢K¹®?%gœL¡v6?uŸæS§?\†ˆÒmfÞ?ï¶0UÞ-ó?vdؐGI?g¿³G·B?dGvQe?yûh=ñp?qèә¿·?wC"'?Œì8Ô±?T&ä%ÇûX?cÔ¸üN?‰Y±™
k?‰qükL´?î~îé¾[V?˜¾ÏN«`v?,âgbí?…»Ðñk…?£ÅØÇïÒ½?•ëM/L'?ï^'Ÿ"óV?ABªz˜?P©FXI?Hk¢"ÒÖ?"#:±p"¬?*Jì AGN4FGL J0024.1+2402¿ÓOÍO¦ÀC4äd™ÍÀ:ÅÔɐ¥À<œ!ªt³0@Þ|§E~º@$™Ì¢Û?ÁN«^½û¿q)%ñ£"?°Ù•³%"@V½ÝñL¿ëKYš¦	?çÐP~¿ê¯ ê[S¿Á"Š‹ßœ³¿ßJâ«¿ðUNASNone?ïìAŒÙ»?^<Hqž?4=…lÛn?*†QDîü?a6ÃEm}?]Ï'Šw?ïé zg=?iJ|¤hB?-ºïÑ·A3?<ŒôtâÚ?eÖ¹‰Ô?f؎³ޙ?8«º{?{å¿5âq?[À‹Ï?dL·_È~?‡»yºÂc[?y¬(½'K?ïãð³-?J'ÒSåG ?=7Zdé»?#žƒÝ#G½?hhý;÷ÊI?Iø	æEü?ïâÎuˆ1+?dòÎûæiÑ?BΰYt<Â?:öŸV–E?h}Þ^Žæk?cj?€ÊÈí?ﱚ'ÞÓF?"ë9é=˜R??±¡PJd?PØ'rê¿?'›ÒO¶Ö$?ƒùUÖ¹ô?ïGE¸µ­e?†^×s;Xh?aÌ´i?gï¤È^Ā?"ݲg	¾4?"å=…<W"?ïºhL¤Z?fm!¤< ?Tô"Šµn?D¶±ƒÎ\Á?}È8هe¥?dR[Fi0AGN4FGL J0025.4-4838?ï%Ù¾wÊgÀPú¹©çÀ:ê"ŒòÂÀ<²ÄÍúÊ6@µ·O,´?ý$ÞÚ5?Ï/®™[_?Ñ0ñd†½I?ýèú}	@@eò†ðŸ¿ã%)Ô½\¿ç濇iì-¿Ñ"…=l3¿æÒSŸd^Ï¿á&á¶hÝ9¿ïÿ«çy÷=UNASNone?ïÞQvŒ›§?d8¼÷¥
?Ar6ò‡I?8Ø~(?mQûîIŠ?bêäúeî?ïÑc}†q&?uzm͗†È?F¾Î§! '?OÆ|–…ó?tvgGÝCM?rÓªáddQ?ï@,Âù?…q߈"£6?q{çêA?såývÁ?" þG+(F?ƒ$ÑÁ_Mœ?ïƒTþßïi?ji±þùó\?RÐзšåå?:r&9'ß?ŒÐ¦=o`Ü?i±–HéÂ?ï²YK ½O?uÒÞµb•?T"‰¼ŠØ?H™™¸t}Õ?€×;ñ1ØÙ?t&êÖEB?ï{{£?]
± IØ?\£ñä
å?mn(zék?ŒÝ•ê/?ŒApbÝ?îÁSs‰Sj?u/·:¯Í?{ˆîA4ÕT?}7§Ÿ²? yªÿ²"3?ŒVÌh8?îÀ¡ äã?‡¢ü¢[Ò?`XbB‡J?S@ÆBÛJ?¢ðhyºKÙ?‡WfÝôVBAGN4FGL J0025.5-5936?Ü\«ªÆÆ+ÀL›â.]á]À:úŒð=ëÀ<bēBg"@äù~@±aCç¶]?ʾ=ö°¡?¯Ò_]ނ'?ãÁ¶¹eü@G¦(s<¿èºGúj"ɿᛃ´UÿåØ?\6a¼¿è¬x™nÑo¿ã(¥ߙX¿ç}YÇòryUNASNone?ïã¸<$§?\7|á+?4Ó€+Ç¢?*¬–ÖEÜ?i¶	Šïçí?ZVh;?ï̉Л/é?v&枰é?I´"Û\?P@â—w¯Ž?v—Ô~ç "?sgàÍ'k?ïpŒuòS?}­,šþù?_x·ÉõÊÏ?TwÙ0™ö?íå1ƒÁÒ?|۟781'?ï¥áìCµŒ?cY#áÊHƒ?Ek¬Û?-x
O³Ð?…0Ê=Êg¢?c8RQ½*?ᅬÿù?p¯3[
‹t?@¤QwÚ?2‡>vӆ?~_-ˉèŒ?p%|Xñ~Í?ï~rè'	¹?Ô1öJÍ?W(ïCÓ=?g*ãÕ9DP?~Eƒ¬m=?Œ"õéþ@J?îë"qØú?‹ødí?mµp~ß?c͆ç9?žìÏõÁЪ?ˆ¾°M'ã€?îؑ§Zß?…8ÿÙr*H?^ç¶=å_?Q:<ÅÚX?¡§Ô:—e?…1üxø>ŠAGN4FGL J0026.1-0732¿Ý§5t½'yÀQa 1ί%À;%sW±À< "€,á
@ fÏlå0œ?ý†»¦3ÛÐ?ÎS!¥—(Ñ?¶ cbPJ?ì7p¿°¯‹@rãºzå?íOKÝyn?Ÿj¿çdq>[°U¿¶Šùm¿¡¿ìô$)ªô5?â2ªw7oUNASNone?ï´ßsv!ù?˜¥o§	l?IËoà!»)?Zýëù‹c?+l+€™?—D?JÑ?ïÆ5À
2?z•sR?Q'HÓ׊?XhíW£?x"¦ò-?vAuË(?ï±MY=ù?ï."\‰?l1I7Ò5_?jû枸?˜ã­2)}:?þ«505?ï7\ü7üú?z~μõ¨?n¯_"ÒÏ?YœÙîµ2?•>t›7^?xZY¯H(u?ï'¡Ìª#?œâR5¦å?U4	s¦}É?aƃŽ¸®?ŒÙV`uk?šõÿq€D?ïl´ö?'Ur
¾£w?bBûÚVÐ(?s	…¾d?3ªÄ:?–œëÜÓ?æP£Ô?•ß^V~e?mdºa‰¶Ž?nE{[Pm?£¡e÷ÈÒV?•Óen?íõõKWRˆ?•ÀïÚR?€áL]ÆÖ?u'mb$~?¬hXHµ^C?""v×µ¤‹AGN4FGL J0030.6+0539?íýò•oyœÀLiˁs2'À:5ÆTǏÀ;å¶BFÌm@&›–Ÿ@ßR@>´q?Àª"¾"y¿¨jԊ0p
?â¶Õ^ìŸ{@÷ç,Êc?ÍïRˆ¸ö¬¿è"NÖý¨7¿ìç,­'¿éÜp
¯,¿Àò§è;é¿ï÷íA·ZuUNASNone?ï³ÖH(?•#Æߟy?k~íµì[Á?"íÜóÓ¥C?x³ž‡mÏ?xpñü"?ïÎD¤س?{ãCkæ?NÎÎ%
…?]ÐU1þ‡\?uÔJði4?u–)ƒü3K?ìªÂ\&g?¢á€ŒMð?Ž<¼ùäë¤?‰úÑHÛ±¯?¶âU€À"Ó?¡¤#ŸèT?ïʂ½žX?c¢}&?6`(²«éÛ?*4ZÓ4-:?yXžò‡é?bç~=›/?ï\¾iT#æ?–ôíxÃ?~}Bpòà?¥Á,‰?‰'Äw¹?
$x&Ϛ?ï~8œ¡f?"ŠZS¶õñ?`88}5e?zSV?Œcʪ³Q?/Ý¿îë?ê1FC±/¸?¬'iMü?ŸÝ_ö??"eŠY›ãÝ?Ã?Dä`'<?©KÂ(˜ñ?ïY\ªG^0?ƒúËxI?Upg#a?Rj͓›!µ?"}d>Iåó?ƒ`¥½'l­AGN4FGL J0030.9-3618?îu…íⓀÀSõ¢œwškÀ;¹6‰)	À<꒽ÝEÁ@ ÷"	â­?ýºžavÙ?Ñ RÛÅ
;?™Émœ»	?͖z·]@΀×?ï_;#í?æë"²È?à
.A0÷Å¿â§Qa¿Ý1ð¥¿É°"‡äUNASNone?ïçî	ø??Xì­ŒP=?%ÿ^R«æ?1°¦±?f±ÿìß¼¿?XL8å:1?ïÑuÔÿ‡p?výãò`‹­?Gšv@<ç?Rƒzð˜?tQÆÅlsU?sÁ+*ê?ïxäL'¢&?wÑlHÄ>?[3â¦?ÿ¦?G´,èœ?Ž`p–´w?w7JÇ´í?¸nh`?p|àž¹Z©?L8_	™­é??qEٔ§?ŠTï<—?p
5~ã?ï՗h*Ð}?ieÓ@ɽ?4sZòÑÀ?&ÿfö­?síI:­
?h¤^u×t¨?QKb?žKªÚPò?U¬DÑÊP?h:ĺk3?‰eã­'¸?ŠÅB«%|?ïÿê¨Í6?"v¥ÎâK?aËP¸Œžh?[ ³3º?šF˜ŽÙV†?ƒ¼8t¢~š?îíW1rÇP?ŒÉ¾¥l¶?Uz&¾*I?Rù@¡BsÛ? ~»»»)"?ŒpŤŠD"AGN4FGL J0031.0-2327?ÖÿiÜVqkÀUÃa@OÀ;ž7Åi+À=0ºö
³¸@]]àÛÍq?ùºÿèƒ?ÙÁ½|LØ?èžLa…V@
ù®º"e?þF a3÷¿ïÿãDÞVb?ïþ'AcL«?ƒ,ì6
qò¿âmSà§Ë¿í&ÕVß	æ¿ê«ßí;^UNASNone3FGL J0031.2-2320?쌠W"ü"?¹}B»óR÷?¤	³_¢Ù³?¨€œ"HR?±–#—¯?²¶UB·?íR:¿?½V"œ†W?£Oýf /?±"2IbÑZ?§EŽ\?±4i[Ô¶'?ê·H±t¬¥?¬—^
Îá?±ž	4Äô4? èAF—3?¸§±@š!?¤Yô™îŸ?îŸYé£?Š‰Ã[ᇂ?˜Ê?ۋw/?'#ó¢Á	ò?¡°ïþSx:?u%<k¾Z?ê:ˆ}:œ?¼²š'³à(?²Kš|"[?«aÝÎ?»à°{Õ°Ã?µ¸n1è¯?ëcŒVåêÖ?ÄûܾÌè?®Ӓ1ó?ºPõÑRîd?µÜ'Þ™œ×?»<
C(¹?èÀx…üÉ?±ýºsdï?µŸÒ	¸ë?¤Ce")Sf?Â.6"f©Ø?¬)¶ºj3J?ìÕæà§Ô?©ՙC?œCùŽ}¯ú?'6ÙiÝ?²Fzc£‡g?—NÎñÊpAGN4FGL J0031.5-5648?ëø7ÈsÀN/Y‰ßÀ;0zW´ò»À<Ëo¤Ó‰@ A2û*?þˆåo®?ÌYO<(OT?¼\iãH;?ò@€"С@k–$ÅZ¿íYqýÌI¿Ùc"úÎg׿ۑÙüᨿà}ßÊÖS¿ÔNád‰l¿ïûs¾¾—*UNASNone?ïã܆(M§?ZÍøh«hæ?+Ùç
vô3?"F>Q}¿?jeÛ¢¿?Yî"13?ïãð*Ai?m'þÐû«?5´Àjx?B58IRf›?j:ŒºÙEY?jF''™c?ï…ÚïòŽ?t)tíaž?WkãÐ_Ù?ON†<ní?‹¥Vˆš:K?sŸUF¸?ïɼi¨:F?X¦m¾"¨µ?4⢭"àe? .{3Ú?yÓ ÷=?X`M5{'?ïÆÝg#Е?mÜt=G;Ü?<6j¨¥ºê?/0=Œ MV?zÍå»+Ó?lò­A²?ï¨æ†Š?†Lgú1?If®åó:ö?YÙó»ôü?"0d'm?"ŒÀ×ÆÜæ?ï"kýK'?ƒN@s[å?`@¬.8L?_GA'ƒè?™ª~è?#i?'íÑݶ]?ïkW!$?vý@¸ÏæB?E,IIPÜé?;>­mÓ?'빕ñ?vÑé*GD—AGN4FGL J0032.3-5539?é–C	%SÞÀN á`؇ìÀ<åÏxÀ<ñ#¬­r"@$ïW'.B3?õhB>hñ[?×ñ¿Ë\ŠE?º	Þ%9Ë?ÛB¾@—õ«@#°Ó@¿êð8ÂiF–¿ïˆ!!7Þ?ëjé]Q>â¿ÄGûa@b¿ïéØÖ+?ïâ±pOô4UNASNone?îçYA©‡g?¢ï'b‡lm?G¥É3éä·?OmR_o?¡+Ô€Þ?¢Î‰\×é®?ﱄ'ŽÃ°??y´ï?Z³'xŽ?qÛf5ó'?€H|^µîë?ŠOz*'N?ê"bU¾+?±¼cÈû?p}è€[?y×ûy'xø?Ç-¿3­?±-¼1ç1<?î‰cºÿ3Á?˜»~í9â?H–ðtxlU?C¡T>õ?§h'$ZF?˜®£Y[?ïAyuÈë'?œ¶çëÞ¡?XEØ¿°Ã?aMRñÏô?–OòEœ?›S[D?ïUñK )? <€ªX…]?b—7Èxê?}ëVk—¶¿?'üÚ܄û¨?"¢?@O?ìÔ¿ùpë?¥SÎûS²?o@ƒG,˜D?xÄ´'ùéò?¸_ü¤.&?¥HFÈ°@?ë>®erde?³öò÷8C?Z/lnY9?m¢÷oòY	?ÂÐ琿ͭ?´	¡œãÛAGN4FGL J0034.6+6438¿ÇNÄ:œ+?ý7ú'ص8À9›[ÖÀk•À;hb{[@<©ÏÜ@ø{,Ç?Ã؞<@£?ÄW'afÍ?@yà{Ö:4@‡å‹_š?ïöòl¬Ò¿ÍkàÊÆ¿æٚpY.o¿æ
ë­òí¿å[LVñ¿ïÿöµšUNASNone?åNýdÖTœ?À`&Y8´?Æ³X¢­?'ׄ,;D"?Ôsϝ.?ÀX¦p}Ò¥?â±ÕùØYÚ?ÅÖJYÀe¶?¢î[¦c…?›q	^v΁?Ø>ˆ›s[?Ä»ÔÛU|?çhAŠŽäµ?®öº–é\?¡æ{¡þÅ?'k¹«pÆ?Íå[d~?¬ñ0_gp\?ä0©7Ÿ©?š•y"偄?­Åç
<iî?'à·§S?ÓåðôŽ ®?˜ó6 «ú£?ÙèißhY?Â:?"w?¢	û2Ä?—´Û…×Ü?áë+^ÊÞ?Âðí¾^õÚ?ÑèjÇ
	?ƙcð%¨—?®k×ÿìñ?­›'þ[m?å%~ù|¦?ÇJe«ø¹1?ډÐê¤à0?³ç—v$?±·¾-›ÆO?›÷7ée?à"ÄìX®?´ ³kâ-0?Ս.«}áq?¡£ ]Ìó?»«ôKR?˜ªÞ0:?áÖ3+·¥?¢I–
ÜMIXED4FGL J0035.2-1739?ïôrp_älÀSôÏþ°t§À;–…AÂÀ<Ù¥o±"@!\Ç
Àù/?úËg<O;§?ÒßÝ5¥©?´>ïÔäžP?äYaϨÊ?ïœ,@¥·Š?ï÷òµ"¡ã¿ë¯8gOšr¿ÛöÀ›æûÍ¿Çÿfèle"¿à­ëá$
¿ÑGã¤)ÀnUNASNone?ïËø}™w¥?€ŒŒx':?1nT±"?8xK"%l¡?xòjBJq£?€/Ƶ½+ç?ïž!´cR?ŽÛÙ$áñ(?f=¼m?Ï¿²Zä?'óCg1Š5?"tକ‡?îê/™Ô/ ?'½Ó"úéå?tb‰2Q_'?/\.Ô?¡jx¾?Ù»ÙƖŽ?íý ÖÓû"?'}uá(…?m'Mv¥(¼?WÀ¦:?®UÍ·º^9?Ž¬[k 1ð?ï «:o¬O?‹´P‹%?9ífð®å?9Ññ{°V>?‡Æ(óÞ?‹iÆBD;?ï±Z´	:?¥*ãÔ.?xœ[šô?"	Çò $?™)­‹Y‰
? ¼«æR?î@Ÿ1Ö?˜äx'?y±~v€Ju?r†ƒsö?¨ÉYºÈ?–%Waí"?êhàÎ%V@?¨êšÚ_¨?{ŽŽT•NH?s¬tÛ²?ŀTs…ð?¨õ1Ø=AGN4FGL J0037.2-2653?Ўl¸Ì ÀUµI''>À;¡éhäÅèÀ<¨,¤£¸×@"ðE¢Ìs?ì>vþdŽ?äy(_ð€†?ïäkß÷÷É?ù–wƒÅ?ýû†5ä"h?ïó°0´Ó²¿äÍp@"Õg¿ß{W#ÓCß¿ØÇáÖt@¿ïÿÆTǏ¿Í¥˜¯cÛUNASNone?ï2¬_;q=?ªœ¤²n«?mi'Ä|á?d€¶]Çt?•ýS¾ž)Ú?ªŒ–.ˆ²?ïƒÛ*?­«Ö¢­wD?'nK§9:—?£:¼4;Ur?–&	ÅtÀ|?¢‹ØÿŸ­¼?í/i&V£G?¢‡"ºê?—ƒ[JƦ,?ãÀ"R6ð?°£ßùOa½?Ÿt'³'_'?ë‹àê¢0þ?«aŽ+Љ?qéàVàî?o;B͍Bš?ÁA-S—6?«w^:&?î¥må᛼?¤ã§ÐV(²?€Ã°Ðü?y"]ù1'?¡x5 ê©~?£Ûc¿GG?Õ"?·pHl1T×?é ÇҐ?£™?0p?¨…î̙$?²9SSê+æ?ìD—~XÂÜ?§vÿ©tˆ?˜òUî€q?'âù">?·ž®­š0?¤'ÕQ??è'Óæ¶F½?»äyšS[z?h>íP¥à?sb¸è,V?ÍR{hè2?»ò]®îAGN4FGL J0039.1+6257¿á¤¼"ÙÛ?¿4GÛ5ñ)À9Xº'Gm}À;ß|ÊUú@oeÉÞZê?þ|óÁ-\Z?¾Í³ýsß?áú|2€…Ì@ Üa•FN@åÄè4Ý¿áP"G!ý¿Ú祖'R¿ÈëJw—¿äÉ"=—*¿ï6©Àd¿í ˆ JxIUNASNone3FGL J0039.3+6256?"TÖè¢ÊÔ?‡@"Õµ?îþ5Ì%ï?›û¸š&6"?–Û
wúÈ?"ŸÀ>ïÁ?™æð2¯4?¥`æ=ÄÙ$?âË7ü˜?Æ};jf ?؈ðn?Åä ;êŠ?£Ð|ŽrÍ?—º ;©?ëZx–Œo?©£œûz•?»Cý
é?¥Q±‰¶ˆÏ?½^îp
÷?˜2nŠÆD?âÚ·Þ(??ªÇYøI
?Òô#	ç¬Ä?¦ÆwF~+¹?zŒÑ(‹î@?ußjœ£ ?îîW"?‰È?šLÅñàYQ?›'çs—&x?–&N)uô?ˆJªÀÙÌ?"ÒÎÑ@?âdØlh3?Ì_žÊÆ&?ÚsùÑ+šý?Ìٜ­¹ü?'¡©S8Õ?ˆ:½ÇõmB?ì¦ã/ÔrÍ?¥"mœx`?¶ |-jIß?£Y¶H´¡H?£<(n@÷Ø?…ÿ¬.Wè[?ä·ŠŠ!?±â5˜"ì?ÕzA'´ÙD?°Ì{¾ô9QPSR4FGL J0039.7+4203?ÕÒ³'À4Áæ>ŽÀ;4ebZhÀ<yÏÛu<@È8ªky@ãp¥"‰g?Æ~ÈÈ[N?—Œ|ù?Ò¤_۲÷@)N^³¿Ûè®àR»¿ÊCBtï–%¿êbÙð!¿áîmØJ¯¿à?ûÞ]Bü¿ðUNASNone?ïǃ¶³ø?p"²XÁ…ñ?BѾ
ë?5_¤NKY<?yä6þ§5?o&yˆ}X?ïÓM¯á.¯?q6ªâCbõ?AVÞ ;b?JûV
N"•?t.L[Z¿?oE1`á ?ïeÇýQœL?}{+׋¢ú?dñKɍkN?`¥¸KÄï?¨ÖÝΦ?zû)¨W9?ï³ØÌB?\zbé	<?L&¦©,7?0®aç_­?Gd¶j ?\¿-[éš?ïÖ)ÂÇ?€L9	¦ë?Uӗཋ?H¼Á«?‰ê%ñd?C"	%×?ï~‡	ýh?Œx'kŠ®?SÞ{¦ž×?cŸ¦3'÷ç?ân
"€??Š^¼ª¾ü?îìŠ2Q¡?‰äƒvcË?ppO|ù¨‰?jêþVS¿?žR¥×O
®?‡ÉeЄá?ï¯í"Ð?{g‡u@#%?ežR¼<"?Rʘ¶`÷×?šæN›Gn?zþ'$ÞçAAGN4FGL J0040.2-2725?F¨'sÀUßµà÷üüÀ;BH­î»4À<|ڀ·@jõ['@‡wÞ]îÉ?Å^j™{炿ª Xz•rn?ãö«ù®r?ùÜÚ
Òüg?ïÿýaw¿êÖa +n™¿æƲ×XA
¿Ú~YÝA¿ïÿã_¶Hý¿µ	-%RUNASNone?í÷ô_Û)S?ÈZæÀé¿¢?Hº­æcÜ?I{N]HP§?°ç§k)Ê?È\Úù'¯À?ïè$–§?«©	…,'»?sé
5§?‡áÚp¼e'?—…8ª´?§ómx
Ð?í@Šû'S?¦9ÅêøŠT?~8¨ÌÀ?'˜–†_<?´–†?¥ÄúZúw€?Ðw?}[§Ïr¤?pw:—&1ù?ZYÆ:L…&?™°@YtV?{W,Ë.Îà?î[éžhÊ?ÁW)v¶?[×&'ù¬˜?` gƋ\?©b¬çaö?ÀîF7O€$?î¤ì^¦?·³ðÒ5xz?R%Îï…?˜±!sãÀ?©ñ0qqcC?µAžK ‹?í–[òõ?¦1c¦øº­?~Vü"Tä?¿­¸á·?µåÝ_¯!?¥ÇîÞÈâW?ìë«V§ÎÞ?¥e]Z´?Œ†Ú8ëåß?âM¥?µÊÉÍÒ?œ0>¬Ñ_AGN4FGL J0040.7-7157¿éÐsa˜TÀF'³¿µÀ:ëHɝmÀ<±'¥‰'å@ ¥×Û?ý%=§*|?Ì&ÝåMø?ÕI7º@fÚå"Cï?ùš¥]G.?ä)€,
¿ïA["Ì´?é±Ç2ŠA¿áPÍ ¿æh›ÊÌA¿äÀ;#Â|èUNASNone?ïŸ!œž6?OÁ:·Ã?Rp¸/¡û2?FccX"4¾?…éú›±?}Åc*«}?î]"cAa?®:År?u¢»Îš$?"N˜ø¡?¢ÉaC•f?§ãdžWr?îgóì÷9³?™[2úªàÒ?'d‹èÒw?'žÚ[`ºß?¤çž9…jŠ?–y`ï"?ëSaJäø?›S¯|\ì?˜ŸB|…?…}íå¢æÝ?¿aÐû÷¡?˜òâP»°û?ï(H¾,Bv?'dl"'nŽ?h@\*g ?`DðwZU:?—îܹvP6?Ÿ;aXt0?ëÞڂ†ÇI?¿ï·æê?¡L5!·«?¬–BøK?¸c'Äb?·Ö8r—Š?írE»².w?£ŽÂ
À?‡$=x»»s?†â½ ´z?±‰Ju|ÖV?¡Lú©…É#?åÔÔ`ÈuX?°ëòšcYq?£ó'
Š1B?™ÿÉào}"?Ñ×æý‹Â¨?°lázÛXAGN4FGL J0045.8-1324¿àÉ+n)¨ÀS
¥¹bŒ½À;§/F>¨²À<ò×;»—ñ@ rj Z=Ž?è×ÄýËrZ?ñ')bÏÙ?ì/"YÒÚ?úÀ?ö@Wÿ÷òjk¿î'ËâA(>?ïþCÒ½§–¿ìCʟöÕà?Æ#ˆIe$¿æÅ&p­¿ïþz#²Œ°UNASNone?ïu#8
Ö?Žqœ½tñî?XÓÈiè³R?RŒÂò¯,?¥>3.?šÿQ,¹	?ïÊËÁ<©\?'ttn®]È?S&ËæÛ?ik–¹z?uÐlTí>?|å¤Ë?î>§/¯E'?šÓ›}\g®?"à*͉
U?†xIó^q?¦Ý'M]çù?—‡@´L¹œ?ï%#| ©G?…Šœ•fG÷?N±‡ifÿ<?V*1Ï×S?šf3ð¸?…›õ€Â€?ï.¢t€ý¹?–ä.Áž`?s1;é4Á?q^ÛS2?•_k¢ص?•W˯EœO?ïi{ãL?œbý_ÈK?hÚù'΃?…ÎæqRlx?eâærBñ?•m‹Š…F?íŸC‹´ÃZ?¡ÈËلV—?‡êœÈ,'?Šß·gB‡?°¢œÆ™?ŸÁ…©Ÿ6—?î·ñW›?›ˆÞ½ð?F_™TÒ?d±­ƒN³%?¤5Óqb¶?›]YÞ~âAGN4FGL J0045.9-2021?áÔ?cSrªÀTÇƧÀ;2/Ú¹šÀ<Ƨ?tŠ@ 5jE8?þõÄ}î?Èüí¦â'?¦GáýÛ9?áíÜçÍS@‡
íC峿îåNCZ?ïô¬ç#¿ânZ†^Sr¿àL0Z:ß¿Ô&2™°?οêT^/
ZUNASNone?ï©ÅcvòÑ?§¢èâQû?NòÍÓfÒ?qñ?olús?ƒŸz@zNê?¤ì!DÖñ)?ïâ§Rûáž?o¦¿•¬M?6ç	§Z4Ç?CT¬×C[:?j{ˬ×?lprær×`?ïƒL"V‰z?sñÕsN&5?ZX§+Àˆ?Sötöª÷O?‹ëP/÷ˆ?r÷÷ËAP?ïÅ]>–àú?[T$Oc?B+lÙÆb?-N	÷Ùß?{[GÇej?ZÚcåâÛH?ïÁü

[D?wHÿ*͎?KÖÍDÅÞá?Eú+MѪ~?{‡!j[…?u•Âqš`?ï¦â4	"K?ˆ"#žŸü?L,'&™o]?^c/Gø.?""©çR[®?†Ø«Žtފ?ï+¯"?ï+ŠˆÍ?`óx7h.å?WÎ
GóÕì?˜ý+¶Ó?4]ª"N?ïq+ë…
Š?v•sν•ˆ?Q³`†ÿÁG?F•X‹rp?¿L"ÞŽ¦?vUCú»ÓlAGN4FGL J0046.7-7048¿Ô®×˜F¢ÀG'ž@ÈG,À;œ¥R4€À<ÒÆ»:Ô@Ӑš—@¸j$aY?ÇÖÎûtU¿¨ÍÆᕦ?â³þÕ]•@¢Äþ¢1ï¿ïü]Ä?ït£`Aß¿çÄyA¿àèõW/'¾¿ïþ5Å´ª—?ïöÇ<jšUNASNone?ï±V;m`Î?{ŒŽ
ah?`Ž‡^Wõò?YR(oùuÂ?
žœãN?x÷CtÇE?ï«øÏ4?^7m%"‹?WâÇC°i?_­–òçeð?'B©éí#?z&ú}ýŒS?îS-weé?šÝÚì>9ô?~Z@j·¯ˆ?ìÐõÉG?§à€¸ëý?™¸»Ç°?ïyw‡˜]?q:RkTÞ?cQèzÛ?O¥%¯N"€?‡Í("x?pKáE æÀ?ïw'"#bÓ?ˆ%¯[¯þ?p™dd¢?iÓIÝ%g?‰Îè6ÞÚ?…ßVC+ï_?ï%Ðqûx?—Á4~'õC?e™—]ڜ³?r³€O
?˜'¾Öam{?•vcÉ#'?í½¹Ca? 'qŸ-?}/(«ÕI?-@'-ÊØ?°DÏ«KA?ž°¶mo,#?î€Õ鉥?'eéC?|±ºÊ,8·?rF£" ‰:?¤hËIÙ¬ž?ÓVÆä•AGN4FGL J0048.6-6347¿Ñ¤L`*ãÀJªÄÑ¢À:ÇK^£#†À<Çdl'"Ó@)?ý<Aÿ~Ñ?ÇÎÔcïé‡?ÚèŸ%ʔä@¦Kaþ"@.ï\ڗ¿ð?ïÿÿ)@k*¿ÙHÅ×Eî¿ä¿Ä}îB¿èÙXáÃ~ð¿ïû²]µ½½UNASNone3FGL J0048.1-6343?åbØ5qã?É%±¤lR?Ë7g¯U‡`?Âf*ä&¨?¾znú\&?Âô6]'ð?꺐<×)?ÆkfyöTõ?ºª_œj%Û?ÀFڋb…l?µ?ËâY?µ²ñ¡õ?á^tßê¦?´ÿ‹À™áß?ÔË<|»šÿ?´n
F1	/?Àñ!3	l?¨3hnE±O?ìiìMâr?"'Úu¾m?«Õ[9'7(?‹ì¸5Í'¢?­Žjֈ³?†·¨Œ÷UÕ?á¿چsÍ?Æ«''âv?ÓVÔ½ÜïÛ?ÄòÊ9–ñì?ÂUß,Q?ÁÌ"Øȹ?å¢)	'ŠÍ?˅Ç'¤è5?ŕJPAr!?ž‡Ç€À?Ãâ‹ bª?¾Ö˜ú¤?Û*€HÝ?¶Z	¦ÓÜ?Ü/
¶ÄD5?·ÙúŠV"?ÁLãþ— ?ªd)	žQ?èþöw:?¦e¤2o€ü?·›ÕÉûI? p¤â/Üþ?À6;™fÌp?gjm=7qMIXED4FGL J0052.1+6444¿ìB´iót?ýíözE@À9y\–$À;Xfêð¤B@•ËÊï'@è‰͟[?ƪH(äj?Ñ-P›#•@Ý ×ç?öؤ^™"d¿Ô=ՃT³¶?éµ{âÏm'¿ß§›š¥³-¿ên¶—b&¿ëRæ÷ñ=Å¿ïݥ̈́'±UNASNone3FGL J0051.6+6445?Ì@[Ó+?½>¨>D€°?'Ãêí ‡?	£'¢Ì¢?èYÉîÝ)"?¾!ëÀ¶qŸ?ÇòFa–Ñ?ÃÖé{"/Ð?Î%9
É<?À*Æ
|&?â¶5,mØ\?Æߔ"eí?Ü{¥×"OŸ?±xÉÎ[Í?µ¾üõF"?žbØHs9È?Þšê…"?±6«ÍG?Ó¦]›ÖN›?¤"Dz_?÷?ÌoÑQÊV?¢
vÉ֐T?ÞMê{€Ì;?¨‹À~dþÀ?°‰¯áÚ{?¤\Yµ7‹±? uULТ¡?œÁƒ|þ›?ìçt®Ü)•?¬5ftkFQ?µet‹Cö?·›e#¾0?ъÁLïz?Ç(™$1k;?äýjéÒ?È¡¢ê¶<?Éå±ÀVò«?ªï›äåÖ?»o|5kØÒ?¢K×·êñ?æ¤	<È;?°F4@??£s(&öË?žð¤º¬[5?Т­º€?¯±ß^xñ?ãßne
?±Oià†w…OTHER4FGL J0054.4-1503?浿~ýÙWÀSz îõÀ;íNäHÀ=]¹ïzw@!'|`Â8?ôÈ͙{f©?âf~x+
?êT•ƒŠcœ@
ŠBä?üù'ó¸¿ïÔwéR?ï}WÎÂ?ïéR‹¾?Ò¹,;È-+¿á‹Y/F>©¿ïøu'ST;UNASNone?ïa5 b?•ê­ý6žŽ?hÇ¿ðŽÿ}?cۜ();Ñ?Àcü·r´?•$>èaíu?ïI&Çü?©þuÀBG?}SƒøUT?1;9тË?tDÇñv?Í‰´?î	f9ߎŠ?œQqWs=ì?'¹	Bì07?Ò$>gˆ"?¦Ä܂;?—}ÙY)d?í¼¨YrY†?–p<2s5P?'5]Qa>?s¾ô§"?¯¨#§Ù›?–'…Æwû?ï³"Yôò?šÛ	x5?yâRnÔø?tÈ:D¶­?—1&(ýˆ?˜)Y*?îGö´ÛG?¶–ÒÇ#Ô?'i:ÀÞ<?¬Ê—´Ú@=?¢K̖¢ív?ª€"Ç:ì¯?í½Z"õ@?£s®³¾%C?•¢Ã+;ח?'KΈÚFÂ?±©d`'`? 1Ü4ã{T?ëä¿À¨YÙ?­	6ÚcŒ?ƒžúÃáYâ?‡Cf·8Ð?¾f"£ïw?­¾ˆî$AGN4FGL J0055.7+4507¿Ö—µqo¯À1½šA_EáÀ;ùÕm…>™À<ý3þ4Må@"¯e3?÷(ÄDhÝ?ß÷×\È­Ù?æS"ÛÈ@a.á"Úî@$m/ƒPW?ïÎT 鄓¿ïÿûÞ]Bü?ïÿ)vP¿ÍkØUÁþh¿Ì¼Õ~@"¿åÓ6þï´®UNASNone?í¤9Ôé?·˜Ÿ#ÀPG?e"s½§îÚ?a9ã³é…ü?²5#¬»1?·€=é·ÂŽ?îûϵÏ?¨ôsA«k?}ãOý©?7…ù	ÞÔ?™&äý7|-?¥®Ú7]S1?옸Ѝîã?¨¿ç*(ïú?y…%µÆqÑ?€bZsÚt?¹¡çM<
?¨l	ˆQä?ìß­õœ#ã?˜g2&3i'?rzŠÏÜ2?bÁqü$ç?·Úî|v¨f?˜øC?ìˆÃ¤k?û?ºß¹0L?}Œ}9÷Q?{Z—&Rõ"?¹Ý‰³rˆ´?¹£T¥Á¥?ío9k(?¹¼~Ǘiû?'žž¬¢¸?£åB)9B?­_	±ÌÄ©?µ"ÍI®Ñ?ë0"yÐ?¯%"s›×W?yžÏržJ?€Ífm¤Ì?Âp÷ O"?¯N¤?çk¸õ~?³âȓîd?z󔽉ßM?zOˆš–]?мÁmYZö?³éwì¢_yAGN4FGL J0057.5+6814¿áð´<ÕjÍ@{ÔÝ<†™À:aGzÕÀ;'Ö*'ò@4¥Ó
ه@ºNz·VC?΃†d9»?¥n…ž?ßiÈñuù@¯>dÐÂ?Á+¡C‡Z¿å­VŸôÒz¿ëŸH˒:¿åTê"H)d¿ëŸ¤À¿"j?µ§\лnÖUNASNone?ão²qpŸi?Áâ øYSÀ?ªOqDÍM?uF¢9oõ?ؓH òm4?ÁÜC¼‡1?ç/^†G?Á`O©BÑ?'ÆöÜÜ2?•U©ïk÷å?ÐtÔk…<É?À&mGV*Ú?ç\£ŠðD²?¯ºôrkõ?œ4¡'›@?ŽcëßM9?ÏÝ°°ó?®ŸÝ?0£~?ëú@|-3P?"ÿˆ³ª'?zÛù¢8?[R¸6Rw?¾€<ˆ=óù?"jŽêŸÏ?Ö,ã•]—,?ÁxûÖòâØ?'<­Í<»?"d¿òì!?ä_ª7Õ?ÁŸÂþl×ð?Þ»E¿•Å?Çkà±cÃ?›ã)¹'»?¥ªþ&#9È?߆‡¤à°Á?Æ@%°¤ß.?ßþª%¿?³nªž?¨˜¤	áµz?•w:iËZ?ÝÐìÔK"Ÿ?³Y¸D_Ê?äaŠ­?ª² þG+(?'>£ì­?{''}+àë?Õ˲'¦ö?ª"B ÌMIXED4FGL J0057.9+6326¿Ú¦Prß?ânù´
3À:{›eK´3À<-yøêb	@"óXˆØ+P?õ~€Ǒ$?̾ywæž?ÌÂy6͜€?ùۑÁ^Á@pUÚ'(c¿æòI~N9Ÿ¿êÊE3÷Å¿æÅp'Iü¿ÔSÈ
L4¿×Á'è|U¼?´°bÞÇv!UNASNone?ë}S¿èX?¹ŸÙþÓI?g#Òé)£_?ahW#âè?Á®!³PqT?¹O ü.L4?Îë°ÎЙF?ÏU%òéþ?'_d¯´†?btö>d?çû–9ùÝ?Ï,-ùk?냙À0X?¨î¡ñ`?x'È_£Ö?q(œZêE?Á14hÅïÁ?¨=Š+îÎ?ìMÇÈùP? 
¥FUaÍ?hºûö§Wð?Z<ßî‹c?¼ËéÖ{Ü? Q3r?ãð{£?Æ¡$=]??r.FÀ}æå?f9ƒ ]t?×ÖP¸Ãð?ƈ)LÞ»?Ç6ÿ0!Zï?Ƅ$T5?{mÍ¢-'‡?"ïeÙ¿Ý?éûd˜c—2?Æz®/[jè?å"ÀÂ&?¶¸üú%ÆD?ˆEñä¤Óá?þmKNß?ÔÂï©E´?¶_ãZ?å|möõâ'?·%]û½A?|¢"eß?xÕÌM›0?ԖшsV?·\.Ύ\¾MIXED4FGL J0058.1+6915¿àþoU½¯@–tŽGVÀ:AVZ¨WÀ;¶o×ÿ/ö@ÊæØf³é@˜±¨ó?Ê$²;üÛ]?Áiànj?ó0¥i±t'@¥Ðȯܧ?ï,pk¢æI¿æÌs 3&H¿åM÷¤ç«u¿évØa´P¿ïÿáåÔ?ïþø™q¥UNASNone?ìËCYh?±êÁî6#ß?…º"ÓC³?'ø	ˆ{?¼ÊVzàñÈ?±{՜%ÑP?çSám\"?ÂêÉ·ïp?œ¢†üS»#?žæ|fÑó?Ð1/ÍÍþ¦?ÁLÍ"üm?éΑ¾·hë?©õ±Ž×?Œ«Ÿ€Ž[?9'aƒJ?Å#iÊ?§àcÆb ??êÎ2—EÆ"?œµöÂJ°?•ÍÃÄoÃù?w "+µ›Ç?Â
})û?šd­^ˆŸ?ç ²3ˆ1?¾Íø±W%?¡ªQü
ÍÅ?Ÿ[kl
?Ï¢±'¬?½æ#µç­ú?۞0:^²?Êj4˜U'?«GÀâGƒ-?±œôÑèY_?à|kãuR4?É;›»ÌŽ'?ã»{ÒÅps?³A<
áåÅ?¬j;k?—*Â^OdÄ?Õ·?²_Ð1Ä?á–Ä|"›Ë?°&ÆÕqI	?¬AÀU`%?•Õ`'»Q?ÙJ>üÙɤ?®½þ7YܶMIXED4FGL J0058.3-4603¿æ£"K™ÀQÁqKœ¶…À;µÀ_@˜À=BûÅ@ô*û×&m?ÿZÊ¡yaì?Ú¢w{?© ÷œY<‡?ÊYƒ©î%@YÅM~¹?ïaì¹ÒE¿ëlÎàM]+¿Î	m&žû-¿ÜSa[ºà¿åG®záH¿¬U½KÐcUNASNone?ïæ'‹×†‡?_Wsÿ(	?)´™êR®?žuPâÂ?h=*yA‡¤?^C%ùÌ¥¯?ïÏaýÿ}W?yŠ¹%&àQ?I#'jÂ4?T/»˜hµU?u*Ž I'—?v!éº
?ï3îžÑh?î镁?V-ü¥ËÃ?VJ"¨ir¸?˜L\¶?Ùl#†ñ5?ï×Ç Ý½'?TžûÏwj?#ºø':¨?h4ï£p¦?s~—²$/(?Tm!gk
›?ïǀOE¸q?q«hÍf?5Œ£…<g?*‹kiiªÛ?zç4%Âv?q@©µ½Þë?ï•1.°±?ŒŠC…þÁ˜?Rj[bW09?bºÖ#dhr?ˆfq/›?‰úñUûÝ?îr'÷#&?—³Ø/¥-?^cøèQ• ?aòö$Zu?§ã¿gëhó?—€hqã°?ï'`MPHu?w]ãkbå)?/nw#7?)öàç»CÞ?Žënô5Ž±?wa4¤RªOAGN4FGL J0059.4-5654?äÐó¹†ÛÀN°ËæÀ9¹Â^´Á=À<êAQÚ@vr€ó@¢ÈY …F?³K¯ÁN>|?É·¾]HZ@Ú­Å@§Ó"ý0¿Ê]%Ÿ÷¬Ÿ¿á¬M P¿ænij&å¿ê–a¡Çæ¿ì6ÎÉ&O¿ïûÛxa:­UNASNone3FGL J0059.1-5701?Åù~?'@èîå}'?'øð¶pÈË?{ÙJë4?s²<¿÷5?jƒ)iª™i?òÜg0?ß"‡
î?n'lfèÉ?{áe
µp?"ù¨(üÄ#?†óÂGP?ï7X|A?9+·ºD?…ö--¦ö?†çñ ©Ÿ?Œ)|¾&É?†ðöQõN?ï9Âù†¶Š?r'Ú}¥b?|"›ß·8¦?`@²à+1?'¢¹Øó.ˆ?n2Ôüa³ü?î¯xÝ-å?™[̸b?š‡Á¼À?"'ʂ\?/B䕼?…}îh4(?îƒÓXÏqd?±¥6¸|Gt?؆eö"?¨÷6¸æËX?Ÿi¼f‹ë?¡´MøKú¬?îݾž?¡‹LИRU?¢ÞÁàÃK?—¿ÑøÁÙe? Ô¿d£Py?–\怕 ??í¦É± ‡±?'¯La¹v?—=™?Ò2?Ós
]ÙÔ?©ô˜e3'Ü?ŒÍÎx /AGN4FGL J0102.0-6240?çk]QûÜkÀK3¡fµÀ;eTÑél@À<à£ó¯5@ N:¶?ý»ed®?Ët˜Ù*S;?¸½ÔakªÉ?ðuøÅyu@*AeûÝ\?ìö—€º¦?ÔüÍÛëx´¿Ú}âïN¿ÚÁ1æ,¿æÕ)' ¿É :Š¿âUNASNone?ïðfôo˜?F"±ëI?!g/Iø½?-ªªDÙ?]°Kȏ€-?Eª¡yR‡?ïÓ¨H*ˆŒ?pÔµ• Ö?B†ÞÏ?Hj¡QÓk$?sÛ—@j?mßqҙ­?"_T
?kc˃'ö$?Táö#GU?=7IÈ5-•?†t:&¦ä¯?jݟmš?ï­L@— ?dªøE6?UǓ6,ÿ"?:¬ÕHµ"?óý'ÀÝ?d.9#º%Ê?ï⿗§sn?WC$×u©B?1Ñý'œ–
?!…FkË
5?k(í'6?V~cñêÝ?‡å<?ˆ5ê'̚?R‡"•¼Åb?`wðã;¨ê?ŠÉR.P>?†FxçÌw?ïS›Ú«K?}ŸE˜¦ƒ?\Ù[Q÷?Y€y¦o£?"¾îýI"{?|µWeñ?ïêDàb^?F—dó6#?g;ëGE¼?V)†($?™Û9ù«:?KÕ¹€úÇAGN4FGL J0102.1+4458?ç¹+¿îºÀ1ܬ¯öÓ1À;@e+ÓÃÀ<®Ó5œš@ )çJ?í)•€r+?ݾ¬
9¤f?ëìjŒeÔp@<¥¢¼@¡¶É€<%¿ï£'Á¹m?áÎϦ›àœ¿éçzBfV÷¿§k®yÐ{ƒ¿âXxgꍿïús™TÐ<UNASNone3FGL J0102.1+4458?îõK'ŠwW?¾>š"39?p<ß	µh\?'È—'fm?GcN«u?ºv
Àš±¿?ï¥k¦ä}:?‰™Žøm'?a×Ááì?q¾ãÿ9½?'/%ÀÚV?…b÷"lPX?îâE–tk?'!Iªoµ?{ö bq+?{Ô¢ã©

?œ¹Å:©J?ùU~Ó?îY\¶_?–¢7Z±¾?sÝâ‡Ûf?kž"E
ª`?§îxL¥œž?%ØøAT:?ï`rôœ?¡¶ŠR?B)?m®ÃcÍÈá?yû7æ@§=?;ÕëšÈb?žŸ,ìßb?îÒ:'î¡Ö?¨w@Ft·?ƒÏ±>± ?O-©uH›?›ÐÕ.Àé²?Ÿ*bŸÊo¬?îDZÆÜ.%?›Ï‰Ãø7Á?€Y#ƒq¶?'ÎmCùÍ?§¤
ÍîÈ?™uL½…̓?íÈOB;?¤˜è<'Ï?ue‡wçÅÝ?x{uO¸þý?¶e®†¬?¤j™vÀAGN4FGL J0102.3+1000¿ÄA1RÀJaä¼­šØÀ:µ¸•Þ#6À<aÁLf
@ œ¢»×1*?ùÙú—á2µ?Ò[ÈRèÛ?Ú³ô#Rë_@˜Cæߞ?ýqÆ^s¨Ä¿Û®ž#/—¿ïÄÜ"«%³?íûÀ«+g¿Ò†É]VF¿æ4½vît¿ä íìEzUNASNone?ïsrˆ‹¢?'Ã	‹4H&?XkZc?M‰Üè«c¤?¼¦´Á0?ãÎÊœ˜?ï);ÿú:ˆ?—&ñ`žÞú?xÚ< éõË?|d`«%-?"¡ðÔ^©"?"wgeN?î*ëÝÍêÉ?œº'z÷¡?ƒÙ_H51?'ý?={Q?¨ZêMºh´?˜úécÞ9?ê"Èùra
? 43rÏÿ}?…±˜€úBO?s/XEÛé5?ÄUo	´?  Ó?îɓÛNs?˜¦Š +¤?q°tl‹Ã?l—B
q{?¡0³Ãd¹Ö?—€"åÚÎ?íÚt›'Ö?²UYa"ã7?Œèñ'?g{? ¬(Ȏ3;?«yìß½?«µGâ!/Á?ìwA՗?§ÚïË9?‹9Mèô©?ˆ2K	qKz?¸ÞÕ(0?¦Q÷j@vÏ?åˆôÍ·?±ŸžÝ6—?Œ³òhñ8Å?"œfJPº?Ô
*@Ejm?±¾žT_óAGN4FGL J0104.6-0818?à$õº_jÀQ»<`ŸÀ;	7·&rÀ<ƒM#ŸA@/x›æ@¡Ñv€?Ö ¡`7x<?µ¶|~UÆ[?àˆÅ †l@½6	Í¿­g:f¿í»Ó`Þj¿Âe?	U>¿äÉùHUÚ'¿ïÿîͨ"ß?ïž^z^ÁUNASNone?ïwڟÐ?‹B…0á?Uȑo<?]7y%Ÿ8¢?PFÒÓ\?Š=Ԇ[w–?ïÂS»]S?~Šc¯Fó?TÓ3ÔýÎ?^õí
7™þ?yÎÁ¼žçl?yJ½h€È?îÑ6tÂZê?"väÈH?‰3)yÉ@?Š¿­eº€*?™?œâŸ(?‹)]$&§?ï£)ä¯?gþ¶hÚ!†?Cù…ö1Û?1uû~‡,?†gsӐ?g.Þº]ýî?ÿ߸|?¡¾"‰ô‰J?aéÿÍ}Z?d£¯e¿g¬?¤ÇÀô9[?¡p4IZR?ïoøS
n(?'œ¦5֝þ?`ñ¦ÐS´ò?qžaŸk6x?Å"
à?ëî¸öO?îI°œ¯<ˆ?–Íj¸wٕ?ŠÔ*4?‹ÿIe"q?¤ä*2û?'úçjÇnö?îóÃ?Ê	=?ˆR+Ž&³n?P«q»â¢U?K<Á)S? >prì¢#?‡àšÐI†AGN4FGL J0106.1+1131¿ïÐLX?©†ÀI–áïsÀÂÀ;ez¤£À<ºÓø:9@ [ž·:¿?ý$™ù;?Ò;9\B 6?ÐX9™…x?ùO¡(TH@ç`Õ®?ë<7Þé"é¿ïþôœõn­?ïóeRj0 ¿èä‡Ôu7»¿Æek"£'¿ðUNASNone?ï¨ê»±W¸?¥q•8sÕ^?SPu‰}w?€¨›$i-?ƒ[Bm!9`?¡çrJ¸D†?ï¡Ç÷œ?'Ê€'z?\¬hv´ƒÕ?h…O.—:??ƒø«åƒøR?'…ä‹#m?î#aØÑג?œ·OF–Â?pÎ+oŽ?uø·‡!d,?«°‰?›û·&N?ïNÃÓ1žf?yõ:>"40?;¤‹?äyH?4Æ ¡8\?•¸ójà‰?y°ß¯«³?ïaMvÅ?•¥½kmI?_˜²uQöv?\ˆ5Z34?'ÜÅø¤h?"ßZÏ÷}?ï/¥m	Û?ó¬UKŒ?c_¹Ó4?wÒñ`N?—Ÿrϔ:?›oÚû±C?ì"Ã?Ÿ?¥G®>'
?xÁŸ>î?}k{ÞёÃ?¹ÍÌn´z?¥v"ÅGŠ?î	5XD÷?™VEhH?Gÿ§ ?JÓo2ª?¯³‹•ò\?™=÷*›AGN4FGL J0112.0+3442¿ÞU¸€†ðlÀ;úÞ]	À;/6oþ•À<µS,;d@Q#RŸÊ?ÿ×_f˜?ÙüxŒØ"?Þáp}–ƒ»?üÞΌÀmC@
?ىʿî´¡'¢?クAûM¿ÞÙ§{¯xÔ¿ä ‹Ær?¸¿ïÿ«çy÷=?ïüK_ÏÉVUNASNone?ï£;}üÒp?{ƒ³}?K½?ulš_¼
?n½œAå^±?xõ¦®'·©?q€ä-zm?ïTÆJ'¦?' ­¦j-2?sjMâp'?zw"Ý/'? $)Ô0?‰DՈbX?îË;þ?šÊ–×u?˜Ýqyƒ¾U?'‰&z€3H?£t"¥Ò¥?'FÚf»š?ï(£×¾¡?ym ¾è7Ö?y)©né4¿?bšDVG"?"¥¡(ò´?uX>.ˆ¯_?ï)Í´±Ö…?'û)Qi?Ñ¯ø&?ˆÑ!!6&E?…þÁBú¯?~7ˆ¾'0ü?íþÎÜ
q?®·Âä—D?‰ÜîùŠ?™'NJ¼³¯?©ÑËրöM?§LÂlÊÏ4?ìò&¸%¡?¡:§Í2? Y¸¸U·ç?"¹dTN?°Bjn÷?š»3~NèÛ?íöÚ'vŠ?"'‹b‡$E?ƒ=ÕÄ/T?w´
ß,Ñ?«Ñîïˆ?'&Ç?EvAGN4FGL J0115.4-2917¿á²bigßÀUvÈ´9XÀ;‡ÚÙÖÀ<äÔÉ'@ µQù#?ûûI·Ùö?Ֆ¬Ÿ…ÁË?Âß#¼r·ƒ?ðZ%Ðt!@Û¨!Ç¥ñ¿ïÿC*!<?ïéÿºùf¿çÀèÞ%d¾¿·½WÓ{"¿ÔÝ[û©Y*¿èÏ^bùUNASNone?ïçKŸ»?]ß6V"~?/a
g¨'?"£ñSô?fï·÷€Œ?\{‡'žE?ïÞ­	óH?q°TJ÷Ì]?;.fÊ:æ?GõòüøÚ"?mí)_/Œ?oepW	ø?ïdڌËLg?€$"_؃?[z`M°~?]gòzTޕ?'¬¶¸Öy3?-Öv˜Å?ﺽÖSÏ?bÓ¿5"¤?;9ÒG›'?)ߎÝÅÖf?€v»èßÔ?bt[çöô?ïÏejµLö?kЬU
g?@Uj]±?3ãQc#'E?vL@
Ï:?j‹É6¿(¥?ïŸ-ÄM;6?ä¡†¡:?Pþܺæ¦T?dÑð|òl?†³G=÷Ê?‹ËXèÖ?îð2v04?ŠTPpM?`›èE§"¨?Zïol-S?Ÿæ44·ƒ?‰º,Û,p?ïNˆ}Nä?ˆ&M½ê?HDZªO¹ù?D´þ(\?•lÍtÇ%?2}M'´AGN4FGL J0116.8+6914?ì{b]±ûª@ì !sOÀ:Eûg¿,À;Ó2ӑâì@®Gp­@=Û	íÀ?Ò`¡üi?éÃãŸw),@Š˜í¢/j?ôå~I‡¿áWR'ú¿ÞHTbWãí¿éÜG^cb¦¿ïýÅÞFî¿ë~Ïu¿â©¬ ÚÁUNASNone3FGL J0116.8+6913?ʊ£Ã¥B?Å?@m8ñ?Ƭ'v­±?ÂÌW(}D?ã²6oÂts?Ê[ïü
s?Ì[Ü¿$?ș$Ô «²?Úd
Å?j?Ë&ïK/†ß?×nØk€E?ħbìª?ß^uÈg|?²À^Ù{È?Ëšy=ƒ™?®H‰=þœ?Ó<ûLÖ·?±pþâ÷ñ?Ä´|HûÇa?¡žl}†Ýb?á®á˜"?±a[p±F?ÒGþªH*?ª
ýÑo?ÁÚ$›1#?¾A;3²´ô?Ë@²yܲ??Ä׀˜Ik?ä¹J:¥‡'?ÈÎ7/
¬?³‰©ÇÆ?¼å·e1ˆ?áª(˜4Ù?η°gÞ­í?×ÉDŠ§
?ʕ2,æF?×J'ˆ|ˆ3?³£óӋ}®?Ò*©µ#@?³hØe(l?֋.Â`7M?´"‡iºZ?£l
¤¶â?ŠõáO-F?äŠ2×ÔÎà?¸Ÿ¯CùÒ?Ô~.¡Ëd?¶âiCÊáäMIXED4FGL J0118.3-6008?¥´Šê1ëÀLUA [ÀÀ;Ëô_¹À<Üò@úœ@¹±Y¤·@&Š"lXï?ʇSÆы#?Ǖb¨@ÑV?ü°Í'eŸ—@m-Dܨã¿ï"Eg]Ñ?ïÆlËÛ5E¿áÅ|vs#ä¿àހ("Y¿êͶ±Æa¿ïÿ¼®q—óUNASNone?ïì'³4d?u"æç'.?FŠ§¿<…«?HÑ°_¶?[¶mÿ?t€×Œá}È?ï溌Xhw?l8͸œ?6<ÑÒ_¸N?C¯Fˆ´FÕ?f}Ù§(0÷?h·xòAê?ïŒÄ›>Ï
?'ïéÀÏ?hó]¾JË¥?sT
ÝîL?†'»:)ý?~"sY«Md?ïÝÉ$ÝÁ"?M«;ˆA4_?P%ýRï?2ñFZ?j*H]þÂ?JFd³—6?ïÕI¢¥?wx>|¨Í?]LT…~Ä?`4´ß¿?lVÂeßè'?pÎÙþtËÀ?ï´QŽ½ó?ƒÐ›&L?Hq`XòíÃ?Y?̨ Å?x•š0ðD?þ_uí&8?ïLmÈÊ"'?ˆl§Àp?{?q›ág‰?x\}*·\x?',ŸæÒÁà?"óQ¬?ﵧ0¨`Ô?g0UYœ?]$+V¤ ?JZڒ†»ñ?}ã\ï¹È£?dÄ¡4¼JAGN4FGL J0120.1+0505¿Þ»¥ ûÀL…£~õ©À;1bZh+cÀ<aG¾Ûr'@Uë²;|@ÿí¦a(9?Äõ¹NjÇ¿¸¼öëÚ.?òÑ8×·âZ@¨«B8‰´¿Á1³VY(¿íáqŸ¿á_ã*cǿ⼫™Ÿ¿çª£	"¾¿ïÿ¤DîUNASNone?ïU¹q—?§/VºëZ?b.
÷êÔ? {Óþø̎?"¬žÒé? ƒqX»?ï¼:§4§?}7ëäsZ?Tî9àʦD?^ÊÕºPÛ$?|ÄTO¯âÿ?wâÎ44žÆ?îï ÝõX?":Gv!Ÿ?cÈêù^b?hQÁAW?Ÿ¦Ž‰@/?"~æ'´?ïu…Ÿ€}-?pÅ%é:˜
?O»]Nò'?9ÔÖ@ÛxW?W0PÒA?peÎg¥Ð?î$±·êßÕ?²™<#Lý?i
¯ù-Ü
?k¾Câè?¬$9}÷'ù?²>ÈQÐÈ©?ïc¡^£¾%?"ƒq.€?_µ÷–J"Ú?l/6&=9?'t·?'P¤iHœ?íôu¶÷‰ ?Ÿoª.}œ?pûöÖ 1?o]^9E?®™%³÷F|?Ÿ5q?ÍU?î 1#lj?'3²Ú¿Eÿ?k°è˜Õ?aX)ÝØ?¬L'ÇÉX?'ÈþŒ"6AGN4FGL J0120.2-7944?îÚÑ4€kÀB¦>-b9À:ÛWvšÙÀ<-"¶³…Ô@L>7±@®åD'×?ÃЀ¶sÄô¿·gɽέ"?øʶ!œÁ@BÏÁ+?ïÖ%œq»¿ê>
A¢a¿¿äè%þÂ=R¿écÑÌk¿ÊÉ>!ù¤ò¿ã+ÕÁh¼UNASNone?ï×Âãٞ?˜}`k5¼?C¾0å-Ã?WW·j›šr?ŠŽ,5å€}?—‡íØ\¹D?t(hK?"Q¥ô¾ä?^÷…§2Æ?n
þÃ`X®?ƒtr=>4Ó?]ôo?î*EßïO•?Ÿ	é]T;?gs »ŽÅV?aјÎ~$?«äoñHã?žÍsQ5›¦?ï¸K#ÐûÂ?e&/	ÇðÀ?8uzpñây?+±Œå¯QŸ?)‹;HZ¬?dqÚFN˜?î ü^Þ?´¸xfu?YÐeí÷h"?[ u'Š¸Ÿ?­!¼‹-Ù?³Éº¹Bäÿ?ïTÆMN4?šöﯧÄ?k2yîd<b?~ñ=éqR'?šoÿ"äî?—
rM9©?ëÑ04;?¯ÃÚMÓm\?}3¤â•éc?xQòUèRÜ?¿£D×å•?¯HF®¤¾r?îü&þDó?‰ËM¨<e?VÁ‹Þ?QËRXýD&?ŸSn·Ð?‰2ðQ¾AGN4FGL J0122.4+1034¿ï¤ªUáVÀIÇ:Þ"_¦À;—KÔèëÀ<È[Q_n%@"5Ï`ûÃZ?÷{Ãà•®?ÔÔÈ#š¹Õ?Ôwã¼R?ÿC;¾òïv@aƒ~ûÉ¿ë-Óî'¿ïÿÿ>¹ú?ïÿç@ìYZ?Ô1ÄPÈÅ¿Ýbí`>¿ÖöçþV‡¡UNASNone?ïœX›?†,´ä¯´¼?A,Ã];r?3?²ÂGn?‡ê]œâP!?…öW(¾Œ®?ï»<à
ÏÕ?~×ÁM/ú?RL«À:Õ­?]ÝWŽN8P?}Îdè½H?yOëñB\x?í''µ'GJ?¦yÝðV}?g#ÉvtZ?s¿":‡œ?¶
YŠG݈?¦^ÏÊ&V
?ï9æ"*Å?'^Ex4»
?=•}Æ9Ü?0qïÎI]?BmE¥<?'M®ÔÕ2	?ïUۑ=¿?"¬Ý8íÁÁ?PzÛfà?GàþŠ'$?"Bö0º?"]SÈH?ï_ìdþÃ?'vOtzÖ?Yˆ@=Nä?iùâ!ý9ª?'w>wu\—?çÑ=¨_¹?ìnfúØEH?§fh^?h/=á´#×?uÛ¸mX"?»ËN:©&Þ?§Mmëò«#?í~ŒÌÆ[ˆ? [cl?N§%…FŸ2?OÈvêا}?³ÎKMTsT? _é▿sAGN4FGL J0125.3+6820?í|q+Ö@³çÑ5ZÀ9ÛîùûÀ;x¡L'H@¥§Yޙ@´hqH?ÓL.!%"?Ðü^ØP@¼½‹j@&¼<
L?ïÙº`ú?ÎGŸ{ÛË¿ê×2K¬¦½¿åÁ'¶ÿ.¿èЩôg¿ïüuÁù	AUNASNone?êw{1Øë?·ÊÒ':èš?£M¥Øä€?¡+À<	Š\?ÁNѐ<3ô?´ÇÌ4…õv?ßø?QéF?Æ'5ÏŦ?¸gÔÕ5Ð<?³‡2'8!;?Ùíû‹|‹?™-,Uk?å´Þ@è}'?¯?Ãþ_&?²Á#s¾ë? nbƒ3ÏÜ?ÏËõCZë?ªéC™`M?äΩ€íPP?¤ÚÆe?Á&1Ç<-ò?Uç"Ù~R?˟(5Î?¢Z™]ƒ?à{`A?ÄqÆ\×W¦?ËJïäDÓ?ÂÀµ×Ç?Ñ;…½?Á¦—䍳²?ÌAIêbg‡?ÂóÖÚu`?ÇÉG:Ú¥?ÂAþõ`a6?âýl³˜¯u?Äjz?I†?Ù­öçí(?±ÝsÂë-¨?ÄÙáâwrÂ?­`æ[Õmú?ÛåÜYw?²m&%nÿ†?Õ#Ɉʔc?­ž#W@?Ð8öRúp@?µ\+Uí?Ú£@$:û\?´~.ÎopCMIXED4FGL J0125.9-6303?àn\XèÆËÀJÐ\
V›À;D}¿H€À<Þ\)̂$@¡·â@ǧ¡š?Æ®^øˆèF?•ECV1?ѧa5úä@•èÞ%?샮uɱ¿â/-êôÖ¿è"·õ¥3+¿ÜCÄûÈõ¿å Ž¶È¥¿ÝVÁÃ.hsUNASNone?ïÛaŽÿüi?—X¯HÌZ^?>jdÍKq?`°"ïGÞ×?ph'"Efõ?•FoyUCŽ?ïÅߊê:?uk«úa1?K–ÀH±š?Q;9ú¾Ú?ybzî8¥?r[mÃã©7?ïƒpôù€y?q¤hŽƒ?_àe"˜?RIÑ+4?‹3†Íá‹%?pp°Ú7u`?ïÆj—šÞ5?VyCQP7 ?Q¯º90?2·` ®E?xfˆ3Žwz?Uˆ¶q
'Î?ïɐéáth?kû½¼
?Gs5?¦]¨?9:	\úÛN?xI$f¿«?jJ·'¼t?ïlw9>ÝX?J€¦_?Wo¢ôö	?c)ïE¨?Í?ú§{}¦?Œ÷zEL'"?ï,ŒØëéó?€¸¼Ã?h?g"±ôú?^Æeµ}"?—}ΜažK?~^¬X%@?ïPþòR²?tõó[Œ+?hGÁéыÀ?ShÖàL]ˆ?'×)uƒà?tkÎðg€sAGN4FGL J0126.3-6746¿ëp\BpïÀHJä)à¤À<D'À=-®Õߛ@!óhbêÛÖ?÷Æ5µ?ÚZâ9E›ì?҆êCM?÷ĞDú?û/,xƒõC¿ïþ…A¿êvjXŠÜ?ïûÚÂXÖ?À{ÝÆðú¿íƒ>Ò£¦?è	K¾DsÍUNASNone?ïuýÿZú´?‰ôñ¯dê?\QEG%ç?Yß«PðN?ŽöW'Š¢?‡þºÀÇ?fñÈý?‡9Mf€¶ ?añÄD ?iŒ¥[îå
?†¤r•½¥?'›&u)^³?íGŒÛèk?¢M'Ýt'?˜X€"›û4?"vŒX¦OÚ?¯Zñõ?ŸFä>°?îíe?Ž¥?"%çÏê´?W|–^'»¼?K¢£û¿ â? mÇS(H?ƒÕ©à!´ú?îÒcH¾y'?žTñ™ÁÏÇ?jŠ€
Í–?fhþ?
Tá?¡1#qEÓÏ?60
šåw?ïtyµµ?œ
ßúH}j?kB(õ9Îé?x›
°y¯??›¶ÌU9µ‡?˜×dƒÌΆ?ì½|_¡ü?£}'¥¹Í?•ÈÈ&º?"	l0"?´¡êú¶õ2?¡8*ýzVÃ?ím_Ž'?¢#ŸiدÜ?b´äëÜÅ?e›×øR?¶Þò"ýÜ?¢aÁ›SIAGN4FGL J0126.8+2412?Õp†c9"ÓÀBú€If{_À:4ÿ—$tTÀ<EÔº.@£øÿ%@ƒCÿF?¼®î?Ž5b¿~áè÷¤<?³ðëºù'@êt¼•r¿ß^E"^ǿ䢅›µÓŒ¿èLÒJ»¿ì(S 8"¬¿Ò`P'yl~¿ïþÁÁÖυUNASNone?ï¹#X…äA?±/N³RŽ~?ê©žûp?±1 «PŽ(?LUšlB¹?PÖFE!-à?ïæçr?n]§9šD?/—¨àx
T?@úME¾$?gU܌Ó?l¤¡E˜?ïZÞu
?¦?ŠC
üW&?T€ð¯ÅÊä?Xåzx®?"\"WÓ,Œ?Šûês[)?ïö®ƒ>A?5uá'!­f?¹Lêð4#?+ÂåŒ'?QGdt|?4~¨ré£?ïíQPóú?"j/ðoֈ?JâlðhT?"#‰l"Éb?Wû"Z%?Z+Vnñ?ï®.ç¡?…ã0%1žÑ?@ŒØÔYž?S½rL?ƒh&½«ˆ	?"â´¯ct2?îÇÓ&áŸ?"Ùèþ¬yã?_ŸKý´í!?aA9úVV§?¢'Èo(?"•{Óåˆ?ïåRÎĸ?U­è_•0è?1[iÅöC(?'PÊZ^Ž!?hÄË'"t?T¤¢•xnAGN4FGL J0128.1+7542?íEò®fbé@)ÿ]5e<›À;,$8Äl¬À<žÏœŠå¢@W­~'ù@cYÿOÖØ?؉$Vv"?îš#A΁ƒ@þÚH¶R@ݲ"L*{¿ï‹oÀbV?ïâù)L)¤¿Ü¤K8ãv\¿í8"†<Ń¿ïþ¯çÜô?íHúåäËÇUNASNone?èäf~å
`?°&4-jX?¨t¨é*Áï?£9ãhï?ÆQ;É|,Ä?ÁHô™".?äèxr`"]?Ê^œÎ,sQ?ÍóÞ¥×?Å«sqøÑõ?¼Ö2¯³??·)½ãÃZ?ç'Fj-×e?°R³)ƒI0?¹ûsÇU?¤-[²60?Ĺ,sÓÝ?ªgª²f\?èXãJßïŒ?ª˜D;
›y?ǂÀÚPC?§ËɆÁj?¬fÇ㘑?'x#NÏöí?ãµU÷¥µÔ?Çغ/«?¹5\8ë"?±z§§Á}ù?ÒGý'U7?Åû¨{ùdt?Ø?*Mí"ä?Íùã0#ß?ܧŸÙF$I?ÏKÉiJ?Æ2k³¾o"?À¥&,[õì?âè>bÔW?µŸQV+R6?Ãƨªrsª?¬Š0ù;#?ÐL.æ·}?²)±ÚL?Ýè`Ä»Ü?¶¾þwҏþ?Ù	ԍ"d?¸gˆþ•?Â(#N}€?©4™óX=3MIXED4FGL J0131.7-5346?àw½FÀO*êt}€^À:¿¾Ô¼…WÀ<µâ;ÉÚª@œ,Œ@6&˜ðý?Ñï ´«m×?ќã›EkD?ú:¹¤ÑÜ@×'n®ß¿ÕLýԺؿß]"Y¿ÜYãÜþ¿éâç¡'û¿é,Š'O{¿ 'ðpUNASNone3FGL J0132.1-5340?ïŒÜ)꒹?˜x×
_½i?`|Mïƒq?Tø–²e¿?ˆ©âFn"×?˜7ÿÐϲ?李µz~T?'Žº!ŠM{?`"k󍽮?d°Õ'<¶é?öw•¶©«?~ÓÓÂ?îÍ$0¿n?'r6§|žF?‰ðakCµ?‡"	Wxª?™Ò¾;Òy?Šp"ÏN6Ž?ïRð¹w@º?p¹«äžu?o;–3QžÖ?T+
Ê?'ºvÿÛ?m5-þ"ײ?îÒr'n%r?•ªßþTp?utaƒm}?oÂAn5n? *S{'=²?"Ðƒ'<A?ïåj8¿?œ§4·Â¤€?s/÷ÆøÛÊ?|Ûfì¾Ç¶?™·TÂ.v&?˜ü-?Šã?íö¾¡¢ì?š—Iäùµ?"ÔjzóX?Ž¥à•O´¨?¦)ভÛ?"ðØ=ðÜ?îR–‰U?Œ™†mO¶7?yíàŽº´B?mPäÙ÷ô?§˜ÛZc‹±?Šµîœ§×OAGN4FGL J0132.1-0956¿ïäê{^pÀQ"KâCÀ:>_ïSàÀ<]o`
+Ó@¯Ûbç«Ë@'¤:Œ?²äôQ ?Ô.;&Ǖ@TbeOåñ@	šhÓ(0¡¿×Ŕ~ýŒ¿åŒqȚ8%¿ì†ƒý¦"¿éS>Ïu¿îáGB´°v¿ïóímVD°UNASNone?ïØɧ ºÃ?ió_ëóbŸ?^  0zâ?Væ9Ô»ÅE?h&¼ê?a^Uxv?ï`:XN?™™ýÞ
äj?xi!¶Þ?‰†Õ.¶šÞ?‹¼ë-`
'?ŽEkƒ¬~?í¦S°ûF?¢d†D*»æ?"uï;#Ò?–zÙ?¦ØˆÝR¹³?š·šNlÂ?ïpÜã§?n¾f"ì?wX4Îٌb?]ÃI~>Ãa?ˆ¬È›EÞ?gBÅr"?ï·­ó1ª6?wd?Ëj¹?l¡åöC©?gßàTò?uØg9ïÁ?o¾°¡Æ?îI°S3?±€ï¬/OL?'KȺËA?£ì°<Õ:³?¢â'!yN*?¤ÑªÐJF$?íj5LÒ—?¢Äwó|†?àt8èÓ?–‡òó7x?ªlk~0?›Õ»çTëó?î'C«¦a~?'=€¯‹õ÷?•g3¥OÙ}?ƒ4*¼-£•?¢Ø+o'_d?‰GȖ‡@|AGN4FGL J0133.0+5931¿ê'Oâb؊ÀP!p"À:Æ(Oªb?À;Ó	¢z@ -Zk[mº@ëùŒHx?Âcwž™¿µ§â1¸ß°?õÄÒG`â?þ-°€0?îIDíoڃ¿êd%¿]"¿êŒ77…¨¿äãÉª¿ÝÖt{'H¿Ä™¢}îÃBUNASNone3FGL J0133.3+5930?ãþ¿º¯W¶?Çè6u27?'5"1`û?zl]ò]?×m–ÝbØN?ÇÁá>ýIu?â\±P'à4?Ææ[$z?†WòÈC'	?ž‡Òã5q?ړÝÉZ¦?ÅéÅÖäRÐ?éJÍÀV‹—?«yòÁˆ?R‹&ßôº?…Q2ÛF"©?ÈÊw™$åÏ?ª‹˜-öÃ?è®KT3«K?¦ƒ#ï?r ­öM?kß^˜âq?Ì/¨¤¤d¤?¥÷òUNd?ۍ•¥
ã?Çõ¾—™¨ø?"h€Â¿?‹Cð+û?áñynDÆ?È&o1lV?ÑëUøÉĞ?ÄdS˝çv?‡=ÿŒ^?"ƒ_°²?æ­]òw?Ä-_Ž'm?ãn‹þ\G?²"D´ð(?šº;dTõB?‹Ü²ägtä?×wDM?~?²9üŠ†€?ÚUuõœò?³¤oLÉDH?—!C=QÏ?ŒÐkGä?â:옢¬?´|BÏ;MIXED4FGL J0137.3-3239?îUowuòÀS§ÃÞ灄À;eEW"&À<Ízí(@']gå@àâ-‡"?ÑB	D¢Ff?ÈÕd.'Ü?ó^"ð•)@sÔ
ƒ¼Ž¿ï‰µ@>3—?ï1g`âC¿é<6a»Ü»¿Ì÷iCŸ/¿ð?ïÿÿ" 5•UNASNone?﯎1 OÛ? Ñ"/¹¯?r^Î̅o?Ÿº ¼|âC?uÚ<?"âӇA¡b?ï͍¤:SÛ?ẍ́ÔÝW?P–Lf|'?`—º¼<þ?ušºÌ‡<?sÂ̕¹H?î¥h¦èe?"ùıÞ?ˆ‡¢'hs?ˆŠûÛ¨é¶?Ÿ3¹¿?µãèwl+?ïÐü38?]'ŒÏÁ?Tف»ªY;?B€2IuÈË?rK—¢QÓ?XǪѯž?ï²N"f¡?††Åk)zÀ?qƚ~ÔðÕ?|<)Æ1Ûû?uT>Ts?~têÌàÃx?ïiS.Œkš?–pވ·÷?e<­#'?z‹{NKË?%r–¥'Y?'Øüݖ¬?î‹(聉?›J8å"#Ù?‰Éà?b™è?‡üI½
g?¨ÔÕeêÃí?—"†ºbÊ¢?ïzóôƒõî?{IÌB6ÿ?j»—§CSÑ?b`í~¯±?Š"용?x
|xÍqAGN4FGL J0138.5+0300?ãÝO=âÀLåùð†nÀ;h¯Á#K_À<¾eò£ +@ "ÆÎ1@^	}?Í[PޔËT?ƒu¤5à?«Þˆ6íg@jÒ/6_¿ïÿÿ" 5•?ïÿþó…õ¿á´ò…Ãù¿¿Ô8ؤ}µ¿êD°~b†ˆ?¶²
>GclUNASNone?ïÄÔ~O™Ï?€™¬"'A?QOF' &?TÁv9z?yAï4êç?~OÇ.¾Š?ïá8ñ|ô6?n<é
¡Þu?8½Úy ?D4jê©\?k¯Rûé݌?jÔPcŠ?î¤c þ»?˜BJ÷KÛ´?ƒðÜmŸ?Š v#:? ÒI¸€›Ž?"Þ…ôېˆ?ï·2½?`
 祖œ?Pɀã"xH?6pÕ7Ë	?€&ëEª?^—0Ñã›É?ïŸô¥ŸH?ƒ©o/ü²š?c–½ZŒ¾?aGЕ®yb?ƒJ½Dš?'§öU<?ï¡e30g?‡¨®Q–¦?Môp›dëJ?`z¦nÿ+?…Çl,ýMÄ?…¯C€Ü
?¥pô?–"Èö*H'?zR"zå‡*?'7€×Eô?£ü3;ȁY?"aSø'²Ñ?ïL?[Ö?z+å+?`ƒê8ÎÃ?Q¦Ï˜ã'?"gŸÎiY?yn3½±KÉAGN4FGL J0139.5-2228¿äô~•îOÀSˆtÀœ<âÀ;G-½¨l›À=, ñèH@ÃÞ,ñz¬?øõΞ^$y?Ò ì¹ý?ìÜB 6m@"ÿßHÐ@GYþí¿ïÿtõubƒ?ïöû¿©xµ¿Ë¨qx¾¿ÞÇlüÃ¥¿înX}šŠ…¿ïþœÞGžzUNASNone?ݞNè£ör?Ǧ\¸40×?Úøs"{CÝ?ȈĹq¿û?½¤÷ӃÃ?³€ìÌt÷Ê?ãð½2?ҁ£·2d_?ѵž%",?϶"¿(ä?¹¨óm>f?ºº3­?Ü48•·{œ?µeoÔûÏ­?ÚÍpX$%Ç?µ@G¯¡V?Áü®$H½<?¨P¢ô{k?鴐'Ll?§2"ù®À
?ÀžCÍ_CÝ?¥ ¦Oo?±÷*Þá?'X¯ä‡õ?םF1'Ÿ)?ÅvÛzJÛ?ßJ¬ÍDõ?Ç×#{7âM?Â0u@7Â?·"3öt†?áDÚ¾¹?Ó1¤'g"#?Ô,*}#Ž?ÑhéÅÎM?"@ú(>?Âŕãy?Ô¿JX=Ùª?µ 5´Õ¥³?àBUéÛ??·0v& EÞ?ÅyY÷Üß®?­n}څü?äéfJÔ~?¶‰^†¨c?ʇ`d¢IŸ?µÕÉ3óÉý?ÁÓJ2dg?¥ÝÌÑvÍMIXED4FGL J0140.3+7054?Ò#Åô㹛@ ÔFQóè›À:ÒIì³"À<k{µƒ@!+µg*†'?ûÑòkyÌ?Ϋæã¤T´?Ç3÷©D\{?ôG÷EF[.@ÄøÂôÝ?æ¹úݬC¿é"³ì+6å¿ãËgÝ^ëH¿Ô§ÿê8î¿ÙÓ¡šÀ`¿áP1ZëßUNASNone?íù»(›»Ä?žîf¢É?cÐþ-—É?Q÷?~Ój*?¯'=5E:?ž|š"È!ã?å'xʅäu?ÃրµrA?‹-Øq€'?Œ€c ¿?Ô¥¼g¤Õ?Ã\ZqÄ+?ív2V
ðì?›—skàãU?t£œi8?d¹N'Ô¡?³3‹/¹û?›8&•ž–?í{۟'E×?Š? °¸dÎ?|ƒ¶äDA?`¦Ý¡É¥c?²Xç'×к?Š¶ƒ/+?ê†á—ÎØ?´ ny·$e?tŠÊ@üڒ?d@4ÛÏS?Å@#NÂ8}?´p;';?Ùi9Åjû?ÄejP^oÖ?"¿l";"?›ŽHxVãC?â²ÿgíZ?Ä-­h?é=í[ÛÚ?¬N#nW-?'ŸwJ(‰?r¸åÚ"í?ÉèaP?«Ô_Š¡{ˆ?èÀÈÊ´™¥?£¬@Æ[Óí?%dñFT?€÷ÖÆ_È?Êø:	¢Q_?¤ P%³øþMIXED4FGL J0140.5-4730¿Ð77g}ñ%ÀPÞ]öU\À;ÚVùÀ<¦RFñƒ@ªÅZ'§@<Ö!à$˜?Ô4›þxÁ]?Ã6«¸«Ì?è;†ß؝@ðš$W"¿çñ¦¿òÊ¿å…Âýk%=¿ãhN}¼n[¿èãX_<¦¿ïú
!ыù¿ï&Nyà—UNASNone?ïßT†6‡É?fҍœ"\P?JÇM¼!Ðl?M·¹¿WŒÂ?iù¦šÂL?cSѸí»f?ïÏ?ˆ¯?w—›&´b.?J¼¡|)*Î?TóæY¢F?u$ÌR}u'?sùå^›A?ïn]$b#Ð?€-Ýx^"?jSNÂi÷1?oc¼Pc=?Óã)v0?{՗zF"?ï¼øñmì?^,Ëz¾=b?P6¤¸ñð¶?6:•®;S?}êZO¢l¶?\/BO??ï¨,%f°¨?{{#t¿¾ž?]c+Ué ~?ZiŽÐš2?'H'0—â?wõ3ˆô«?ïu rž$?'(ð¶¢C*?^Rg«0×ü?lÕ9;ƒ?ŽÍ–Zѱ?^"SòU?îð‡ICs?r¼x%\"?y,æq¨«?}">Êä¿Ü?›¤|Jh?‡v:«ç;?ïQLŽ×|\?}€M"K‹e?] СïÜ£?Rü° 2nI?"a œÑ´?|]Y.'ãAGN4FGL J0142.5+6650¿äŸ[žûòï@Ö¬¸ZOÀ:Y§uû.àÀ;nŽ	Bžá@¨³0C"ª@,ʦßi?âä"wy3?âHȐýé¥@¶B9`sÞ@z;×F£R¿êÕb{uA¿Ž oPÅ»¿ç†è‡=vƒ¿ël°Í'Åj¿ç#Ÿ!BðÀ¿ïÿ¥œÝùUNASNone?ãŠbmøñ?ƲüŽu=?¬ªÛê?Î?ª@4K×±è?ÕUß²¤úÃ?Åõrú.Àï?ßtBî£G~?Ç»›:ó4Ú?´Ð8Òòe??´ABš.ü?ÛW®Û¨»S?Ã÷äª,?ãÂgeŒ?²Hyä,Ü?½@iDŵ_?§ù¦Áí˜?ҟÄ+¨N?°@¡€6ÔÐ?àåÚ<y?©Ü Kÿ?¬×"Sž&‹?•ÒzñÒ?ڙY䨝?¨Ü²)$¿è?ÝZ<ö?Ã÷€ô6ô?ÂJÇóãÖÃ?¼_]óü²?ÙËAóф©?Å7õ ç§Ö?Ì`ÿxŠo?Âz×
å¾-?ÆaNãà1?ÃÙ­Ÿ¤ºN?ãO{$l,?Å%¾£?ׄ)ñÒ&?²Սé÷¦?Èzà•pXò?±²ðÿý"?Ü>eÃu­y?´)焒?ÌôÀ4—?¬Ž8žtMC?¯Éz5ÿ€?©îv½?æÆ=åFsà?±ÄÏ[Ö0MIXED4FGL J0144.3+5959¿èw»½¨9À"%B{¦À9Ýv<?AÀ;ŒjýŒˆ@:/&‰+¸@ŒÍ{Hu»?ůŸ)üRÌ?³yéûÜ°?ç@#qPM@J')ÞuÂ?恋ñ:j_¿–ƒaô¼ªì¿çÓ¦¹Ù«¿ëg¾Ö¿èR¬?Ž‹I¿ïúK¹ëUNASNone	?êkIý–?´ð'†°?k²[iØ0?tªæ³QËU?ÅäŸwv{?´Èø*¬M'?ç]ÌåT
Í?ÁQ>îʚæ?|OQwäå?~鱙q?ÐÓ*´•s?Á
ŽS?ès•±á¹?ªÏ©VVø?Ÿ¶øØ¡õ¼?cѨØœ?Ê:ÊT…¥?¨ÈK@—¶?ìI̵®UÇ?"q~Š"Ù?'²Ïì)?q_,kYôu?¹DæWƒÈ?'Œ,eçúö?áó²Ét?Á3Éå?y~Æo'Ø?sÁ1¶Jó ?۳낣™?Áy(Pè6?ÜÓA-ûC‹?È2Ç]L6d?Š´ÓÚþ«Ò?šÙ3×U¹[?á+Œö˜›?Èb¿4U??à+ƒrLþ?²Rî¨^?®e£Ýe,?—û{8…ƒ?Ûè¬gã¥=?²s¿{'­?çDaéKþ?§"Gç	·?¤è8Xi?‹gÙò¾è¢?Í´jY©ÙG?¥øV¨Ù'¤MIXED4FGL J0150.4+4848?䶈µ=À)֊"lXïÀ;•PÔ-êÀ=5²Ñyø@ ÔYM= ?û?ƒ¾f½?Ö19'ò¹?ïöá=@K¡¿	?õ›?¤Á?ïÿFÄ¾¿é9M(¨¿âšýFè?ÎuÎù¢Ãº¿ì
îÛëMÁ¿ðUNASNone3FGL J0149.6+4846?æ¡&`'™?Çc72‡?°¾{-?±s1ýuâ?Ít]uÄ?ÄëEí¹Æ$?ÖݑŠEW'?Ñ[µ€Þjb?ÔP3€­\?Îy›¡M?ÔÒ\B9û?ÊÕ÷¡jQ
?ä¢2\!?²ßÃÙké?Æ#ˆv»7?¬Ô —ïÞ:?ÇS®èÀZ?«òYÃþˆ?ْµIxný?½¼vÜ]ìù?ߙÕëǞ?ÁU±Ã$‡?»MÓ-Ë%"?§lÍoËD+?âøI®°é(?ÉôÙn¤V?µþ{Z§1?µŸ¹Š½*?ԏÍËØä'?È6fÂ4v?ȟ¦Ùž?Ì&
l
{j?ݱf'¦Ó`?Ñݵ'¶?ÕþÆŠ!_?ÎyžÅ†,?â LÒüß?µê·†J¥?ʾ..;§¡?±¸/ÓI—?ÌÀ¡tž&`?±JaçÚ?Á£Ö‹‰ØÔ?·YrMíw&?æ‰Ò»õ?Ɛ"W?Ä4àý†S?»ßÓþüMIXED4FGL J0150.9+1230?î`fF¨RfÀGè>ÕÀ;LK?™sÀ<‡ñS"ÒŠ@ZEÚ)ו@U×DõÓV?ˆ#›»_?¡»
²›R?×W"%ĵ§@Ù¡œrg¿âg¨mqó¿ß
º¨²ç¿çÜ7Hkª¿ä›…AÚ¿ÑYƒÅœØ¿ïÿ`h¤
UNASNone?﵊²1QB?—‡dÿ,G;?<{¬àa#u?2|B·º'¨?¹uÿýF?—™È{tå?ïȜëù\?w¶¶ó ?G[žÈÒXÅ?R"çf€?xÆ©ª}Ö?sí†jº¡c?ïS"V2Þò?ÄõÛÁ^¾?b#àî	é?doÃÉyI?"Jù¶õ?€Êo¶'nÁ?ïǺŽS6Ö?[xD1ú£F?06nÿú?gŚ'*á?{QÎW¨?[>÷B´^?ïYQŒSy¾?ø8ðÞæ?Lь²WÁÀ?C÷$ZSq?"ïBÈYˆ?›ìºñ·?ïqÊ&÷ˆ?Ô߸.R?R£›qÔ7^?aæù~ȑ6?œa†±?ŽrÄ8k»Â?î§É:ϒX?'‹ñ'"…4?lçœ}—äò?kßü9¬àý?£´òŒ5>7? |ðºý?ïFòŒò8¹?}Pûþ?GcûàïÎ?@iy^à¬]?–fŽþ»?}e§-¼¶AGN4FGL J0153.3+5416?ïþ&•¯ÃìÀ	/+f¶À:êo.Œ†À<‹ú©u°@!"6s?þÌœ†³ä?ċÕ`ÅÂ?"oŒ™šµ?ÐGÖ"¶ä-@íîò;œ8¿â'^⎀¿ãvÍòfºI¿äÊÄ°ž™¿ÛþüôâÀ¿âÉUê`o¿Ïu6
GUNASNone?ïŠC‡¶–?€n>@?B"|ˆ[K?8»Ðêi)?ŒFÖJœRÔ?€'ƒH"?ëN î¼O–?·tFupŸ™?Xšft†k;?dv4Æûai?"Gy€
p?·6Zœý2?î5–#\?`?"ªx^?skµv?tãœa:þ'?ª9<SÇU?"©c—þ.²?K'?p­n=@ls?TŽ'[¸±?9îaÿ‰.ù?ŒJšæCÍ?pÁo®­3?îÓe–˜ïa?¢|cÏnxë?T5áŠ0\u?TSa'Ây¨?¢'÷ˆÃ?¢#ôÒª{L?äœ%åí°?Æ\Á¡ö_?`ŠnÀ"e–?rÞrVÚ(?Ö¦ŸW"Ý[?Åí¦â'Q?ë‡éXs´ƒ?£ðm©ò‰?}¨kÁT?v
	›¼¶ä?Àó»pŒŽ?£ŽÄñŽy?înr{"î1?‹*™pNÔ?mÂ`Ec¯ ?_…xd¿—
?§<²>ÕH‰? ù¡vo¹AGN4FGL J0154.6+0051¿ïôÜêëà}ÀMÄq´xBÀ;ÆÙ{0øÆÀ<É·sŸ4
@!³uy/A?ß¡ª	SeÙ?è«@UZ¥h?ïäNÿA"?ü}å#çÆ@†?`"¿áýÞ½ç¿ïÿ<h"?ïÒ¯´ì¿æÖÿöÅě?ÎÌc8°¿ïÍ­ÓïUNASNone?èÓÝ"c	î?ÏÂA²Á¢'?l ©ï®HZ?x™''s?Ì@ÎۚÆ?ϾÁÀÃîÇ?
8W?˜Fsý‰ËI?g'èsfÀ?z²Ü†2E?†ÔâøK?"âËÌ"¬?ìâÆ3U˜?©úoŠ`ó^?"¾j{¢Lk?']Ãœx?ºùO.2å¨?§Ò_Ӎ Þ?ìrÈ/ÀH@?¨O#ÀÙ·\?'â·Yú£L?(o|xޓÛ?¼]Í%7G?¨MK§%ý?èID'™€x?ˁšŸS?…¸`´>Ä3?Œf¦?Ígê?ʵPØXÑ?îõÈ¤7ò?¬¼ÉÅ<?t¤‰nÕ~?Á"(yBw?œ$䪨Ï[?¨B\ò¤k½?êve±yy?°ŠlÄd¤?"I§½‰Y?'v
Ü'™?ý4B@±?¯œÑc]¾?é¥ÃlC?¹?"%ýw?è:7¡Þ?0(áx13‡?ÉeõG•?î?¹>¡9®ÉîAGN4FGL J0156.3-2420¿¬THÎó:ÀRÈÁæ¯ÍÀ:ž¯ñʳÀ<ßŠ>²Ã@&âéê??ý²øE ›?À"8#²â–?ºÆÏãÉé?ünà¾Y"@
kRË)¸¿ïþ¬B鉜?ïû .y¿Öôý"U"¿åv" 'E¿Õ‹¥|§¿ÝªßÃ^UNASNone3FGL J0156.5-2423?ï±¼nÁåÏ?°ÀA(¡6?H
éê5 ?{^—zY‡6?'5®=åœ?¯"`y?ïïùMÅkì?dÉYWaŸ-?'H»¿°‹?8SE"ÑÒ?]$M%óe°?bºšŽjË(?ôZl?{¨:I?V,z:»^,?bzÌ($õÍ?"Qì?•P?yñ…C?ïä^Á×P^?Ib«»²p?'ê¯Ý[9'?JrX%?j""[¤÷?H±ïP¦s?ïßD·Ñ#Z?"#äh³??…ú3¸-?``lË»?lÊ£õ	¤;?'Zö¿¼"n?ïÍl÷Çn¶?}®õ
˜ð?:9¹U¶ÿ?LŁIv?w¥èOƒ–?{é'Ô!5 ?ïl'^¶æÿ?ƒFÃ%<?^¿Ð¡Ø×A?gÂ~Ïy¹?ƒ·$Üè«?',Jp	%?ï¿Dp¥–?e
ÀAûY?7ˆ"£{ä?-\ž–8îz?~ì:ÕVÇ­?d¨IçÌ1AGN4FGL J0158.4+1230¿îÜÊ^'
ÀG"‹—xW*À:Îû­Šè&À<6Îý(µ+@ÔЯZv@9RKý."?ٔ»#6â?éH#à"å'@øÚ¶š[@O°oó?홽 1xÉ¿çd•ÁGÞf¿ïÿÿ" 5•¿ï5A•Ì…?ïÿÿ>¹ú¿ïÿfb4¨~UNASNone?ï:7UÏ?¢j!zܼš?…ˆ9$,è¾?'2Q¶Öì5?'tœwÜ'?œ'ˆjyæ?îó#vNÄ?°q.úL?…ˆq'Îo?œ5"%«p?–×f/"*5?§~~™#'?뽊'?³?§~åñƒŠ?ª¡T<Üîó?Ÿ5Ž_üj?´ÃQK½'?¡mƒE'0À?ï{PË@ýî?'ufØÕÛF?Eh«{>Àø?I0qø ®÷?ÕBoļ'?ùåO'?î>.'Üw?¯´ÏÈ-?y?¡KÝT'¡9?¨N€ðÅ_?•¢s$=`®?8øpÉԐ?íEéG›ŽÖ?¾1má/z?šáAk2½'?¯ëxøMÿÉ?®0ÊÎõåÙ?´tM½·þ?é p¥{òa?¬Òþõg@?³©¢.ÌBÐ?£×µ·qÎ?¿Rئ0&?¥šc;`>´?í[ñ™#Â?­Ñ
ŸZ?r«Þ]øh?~qìÿE'?´³Å/n?«¾H1µEAGN4FGL J0159.0+3313?éÝF"ÑóAÀ;ÎázûÀ;avؤÀ<¢‡~äâm@ YØ&ÈÙ?ÿ'äÓ?ÇiËu´¸?¶eΐò+?ñÏîTÜÑ'@	Ò¯4‹wî?ïíJÖE¿æ¤œ—zÛh¿Õ°¡]ˆF`¿äÁ—½÷¿À¨W{'ò¿ïÿý¡UûŠUNASNone?ïïŠzJ|"?V›tG ?&¬hãø=?"æ)öÜÖ~?^~ÍF6?UV[§Ú?ïÐ=œ»™?r'òÌ°Y?Ap4†¸æ\?KYº:¾"›?u³+2"m?oü}Š·B?ïV3›QÄ?ˆCCõÃÔ?X¸g|ÉO?bèþhɕ§?"¾žžšç?‡ý%˜M¼?ïÀ÷u(1^?`ž¸)ŒW?75êJɖN?# ÀoÐè¸?~淍Û?`Œ"`Ö?ïØWtR"ª?p®F+â̳?>Óm¥"vë?:IÛyaˆ?qçëøÛw?pi	v|?ïƒ'N®Â?‰ ñ¹¬Ž³?NöæÄQc?]9˜ÐpA?FÙ@>,¸?‡˜™þêk?dek{?–Pé«J‰?a&`֞KŸ?jAKÈ×ÿï?¤±³®Ó•?–%ÿ±}?ï3ÒaPÜ?€öÇ»¡œi?Mã-›…ð?BðÊÜFbF?˜–šd.xš?€ûZÖª¾AGN4FGL J0159.8-2234?çXïéÎÇÀRv¢‡~äâÀ;ªðÏ
•À<ëžÈ­ƒ[@ ö=@RU?ö•ÉæhE?à»E¼Cé?ïÌýߔO®@» 'V†õ@9A‡´¿»¿îâáH2Ÿ?ïÁí@	ÛK¿ÔäçßCr?Î$Œç¯|/¿èÁèm<C}¿Úˆ\ÛMC*UNASNone?ï!¥þ=u?¤[}e}Ö?v]öBvy?€-
ü½"9?–3¡¼?¡<DþÝw1?ï6ç8Äþ³?§d0¢§bÅ?ƒ¢¼¸—ˆ‹?Ÿyʝý¿O?Ž£u ϔŽ?"£fþºü-?î¡?.­×-?•JŸ¶›?…
¬'‰t?…Y¯i|«? ©e©"Ó?'ælœ.¡?îŒ)w%Y?'«l~#3›?x/µ§?ª.lÿ#?¦æûÆ6:?°1Γ¨<?íÈÖ,¿H!?²¦£<Ïvó?•r*ͅš¹?—¶³'Ú‹ç?¨¹‡Ëâ'?­Å$ª?î¤dp9p?µÎ!,?–(-w…¾3?ª‡Ý)r\l?£Á¢ùÉíæ?§MÔù¡?íÙE™ÅÁô?Ÿšßºœ:â?‹¢Ú w¹?‰Óϛ?SU?«'ïØòHR?›Zöú%~?뵪7æ: ?ªYÝóµr?œvoÈå·?œn²gŸ5?»N¤Ûõ'?¦âŽUßpAGN4FGL J0202.4+2943¿ì™b½"À>¨
¿v¢õÀ:æëlËvÀ<Œ<´¼4Ï@ϖ‡å<@áa¡Û‡{?Ä¢J˜)¬ø?xÝmÒ¸c?µ·g	úTÅ?þû€'µÊ}?ëUx™]4¿å#¡Å¸¿àwñsuB¢¿ãÉűO˜Å¿Ø˘"Æ£¾¿Ü­Hãs­LUNASNone?ïŸtÅ­Qe?xøP>äœ?J>÷Q?9<×ݖô?†Ú¶'?x$…Á+¡?ï‰G‰×YÄ?…%Qœu" ?`øóì€?dfÜwI–'?‰oýÂL»ü?'yÈ÷]Î?ïmՔ'¿Ÿ?z¢	ÿ?`»y{ታ?X†^˜Ú‰{?-ÞBg™ò?y,ôv}>~?ï¾ôêE?w
 +¾?býÇÆôŠÈ?G5ñÂÄû?œÜ¯$¨?vá$¿ÔA?ï5í'5N?iꉴ?[·ýà{b?M¬·r§¾—?—†Û:ž˜y?Œ#ä	%š?î´'™™f?¢vY ÂB?kn l£–™?uŽPš`¿?£¤]7«¢?¡Š7â©à?îßN¢­òö?
úÛb?j
'&PÉá?b§Žö«:? jCdµŠ‡?‹ ¿þˆ0¼?ìÙdO,Zs?•¶+!v/?z_£ŸDü?h¸wºÓ!?·ŽãMMØÔ?•_œÖaŒgAGN4FGL J0203.9+8120?ïÏ¥ªÒ"¥@2ݨG²F9À;"Îñj;À<ª<"¸@ §/"R
?üBöõ•C?ÒN{ãüa?ѳôC‰A³?ýT£
[£•@!ٻ̿ëÍÂ6Ƽ?ïÌ$Ñp |¿ã¬Þ²þE¿Ç=:ˆ'
Y¿äôdUêî ¿ïþߤ?åÉUNASNone?ïêëu¦Â™?Sk4@vU-?AŠê<`?4"ñqôÆZ?`±ÏÞ«u?PÃQô%H?ïÖŒ
¿Ü?u3ÄZ'á´?L1ų=ÓÅ?V7½Jgœ
?qnBNÉÝ?qÐ7§jt?ï€3Èôý?|•yUšH?d‡8œZÙ?b]
ÿGu?ŠÑ?'?z•]Ëh?ïƒÕ¼×ٓ?f8|£´?lã™W«i?PEa<ôm|?‡ãëBÔr?c…"YP?ïݹðç?az»?Mè3È_!?B°õ#œ|?jÌó0?\ÏædOï,?ï'QŠµâ?Œ4ê80?bÑ[›õ?pçº'ª#?Š·I0_>5?‡Ø9™R»?ï/íǪ_K?"íðõ%O~?l{o'ï?kàö cé?–rÙ¤dË?ƒ-xi4UT?îò"êÇÎO?€»—›ìá?x}U®™Ä)?g×Øïoäê?›Ž-4(—?}¡è21AGN4FGL J0204.7+6656¿Õ,·¿cG@Tâó¾ýÀ9¶ZöƛZÀ;˜í8}@ݪâ`@ؑüí&	?Á °å¹±?Õ›e Á@°Ì¼Õ,?ý0é5_?é²X­@?‹¿Ö\çÙßZ¿äèÈ%ž¿èÚ'Ér¥9¿ïÂ[ßú¦û¿ïþ¼~K	"UNASNone?ÀÇÕíþø?°-îÎõß?ØlP*‡?Â2B-³'Æ?߀¨ð,Uý?Áèԓ\:?ÀäõбŽ?µóe¢»0?۟cÅ°?À·ô¡Z¶¸?Ûî",‰?À֟˜zúa?Ô÷vºØ"½?°ô$ÄI_^?Ѧ UŠöê?°¡VœaÙ?ÙbhïœtY?°ÿKÁ'0?Ì@áD† K?™À#…»ø1?ÚÎyu6ä?¢w$B¸2ø?×ÍÀã4˜8? Ï4t—.?±ÿH5~?Ÿàí!HS?Ù0^lœáM?Ã:6Ûf÷?áEpàÆ\y?ÃB!Qx1"?©±F%ה¢?ªO«×Ut?Þ{kw¶p?Çb^,c¾Ê?ÞNl&;J{?ÆZ¢¾O?Æ¿è«Ùâ?©]-ä‡?Õ8bà¨n?¶Ž	þO‰}?ßg¨Éjö!?·Ñžª»Û?°ª-+˜p`?ˆ=[[¬8?ào™Û*U?ª"	1ÔyÅ?Úö@þ;Ét?¨¿›ÎₕMIXED4FGL J0207.2-1832¿â՚8svÀQ¤Þ*Ã")À;5Ç/ÔÙâÀ<ŒN«^½û@C,[}ª@êB¡e@?ÍSW@Ïh¿wêZ½•ì?§{R[Âsƒ?ónÒHaÔ?êšCb«Eé¿éýöHò¿ßƒ3ü†Î¼¿çŽ"'Ùc´¿ÜÜT^ü噿ïîQ Ü"UNASNone?ﳁë/Áí?—eVŠ¿ü?[úªs07?–+¤™]ü¹?@`Žá5?{*›
OÝX?B•7?Œ'h»ÛW?g!qÜêÓ?s6v‹Vó?"
Rڈ™7?…־͌?îÿ¢ØÉ?ŒˆYƒª?{p\Ӊ?€(lÉjŒM?™/¦EUrï?†¥[Q†ñ¦?Žäðì?Dü@¶]?hﹸ%Qo?Tk¿£då°?¢Èwüg¤?€•\¢p?ïQ±úþ'R? ƒüõð˜À?cʆy;ã)?2>¦	è­?"PoÍûól?K®4¾?ï·côœ?¢!º#¢¨~?u3	åUˆ‰?†|-'W#L?™¼Q)"LN?Ž~ô¬Ù ?îC-÷µ×?•FoaGÿ¯?‡:ûç]?‡ž.u?¥þa†
[?'"+uÿ0?ì*"¯tÍ1?Ÿ0äY#¶?~ëԉ¸…­?rɜhAb?¼¼¥;¨š?ž¡!ÊÁ^ùAGN4FGL J0209.8+2626?ë"Îa<À@›OKD¢À:묊7&À<P{B–~@ÖMô™=@'°Ì¼Õ?Çe¥`ÍX?¥¥
|P™²?Ûe5ŸŸ@†œñû€¿ßDÙ»J¿å$ #!¿æ› ¢ŒÝI¿â}ŠuV¿æcü^ŠÏÒ¿ï×þŽæ¸0UNASNone?ïÐ$Þº=²?kNñ'šp?<V¼7­j¿?)¶0â3?v($æ¯?j¶;mkÌ­?ï¶Mü¯Šê?y('+ÿ?OEß°K‹ó?SÄ@¤É?€x"ÈÏ3§?v?WêÞÁÓ?ï)w·`n?v˜ý¾,!?b‡©Ö¸¿?]ÞÆßËv?‹"ÜÚû¨q?tj˃'8'?ïŒ5$úá2?dcd´û–Ú?\Én'ŠW??xyd
?‰Y"!ãÞ?cxqèçëÐ?ï‡Åû¼Y?@¤¹Á®?Mü6à¯:?@Hs4DI?Œ.½šº1é?~f‡Çª¼?ïy>ZX¼?—®þPj‹?bE,€v½ä?qy-V8£?›2©u"¼?•«\°G@?ï#±‡:á?'Öïéoc?lZD–žA¾?aüj–A5ƒ?—þ†"ô.?e"¥Qð?î¿ÒOºõ¬?'ˆ¾ªùŸ?r%e	?]%bšfäŠ?¡ÂØ|4W@?±58Û7AGN4FGL J0211.5+6219?ïª<6'
^?ìXu—5À9vZYê
À;?®ª@ÒÆÛD)@ã.`e›e?Æ$nŸDÿ9?¸½èƒažÖ?íêsÁ˜¼$?þ¾¬Ÿ/Ü?Ôh`;©ú:¿àâíP¿é"@U¿å<jŸ01v¿íEO?ƒM¨¿ïï¶Ü gUNASNone?Û¯¤=¤?ÇtTA1ó?ÌˆŽ—Mˆ?'ú¬7º¯#?á±E‹‹ ?Çt²w""«?Ø<àÒN}"?Éã~óƒ£l?¢¶´1 a	?Ÿ,Àj¥<?â¶$S¾»_?ÉLy çÂ?އ?"E9?µz Ž +Ô?¬ÆÒêv•ƒ?™§K…zØØ?Ýßæ¢k7?´…Ãe$Yí?áv6Ä/?¦ó&'`Ì;?±S¹$X¸?ŒªDNÈìÂ?ل#-ä•?¥Òš·8×?ÔÏûð¿?Á´KGbPh?—à<ýG¥?ŽT»} èä?å;bp§?Â
±ù{›?ÊWuÆk?ðg?Ãÿ
?ªQG"Žþæ?±€ùªý·?çÅR³½?Å;Ò¯öä_?ÓãO츋³?±i#8Y?±!‹ßÕd·?š3X('iæ?ãê&ÄŠo?²$H âöö?Еøúì?¦»O¦û9Ä?¿]¥É8ÿ·? *\¦ÈK÷?ãÉNÉÍÐ?©Ÿ†?5$CMIXED4FGL J0215.0-5330¿Íš|ÖÈרÀM¸H@áqŸÀ;¤†*QbÀ<ër
—@ 
mý´v?@ßËlÂ?ÂF(XcÄK¿À‰¢«'â?ó]]Äuq@ß&–—²¿éS®2­Ò6¿êµ0-Å5)¿áqô¿Zƒ¿×õ·ý‡Õ¢¿Õãm"BJ'¿ïû¥]:ÉUNASNone?ïÉæ®9(?UÌ]	Ê?IF®!H—Ç?Lœ•'¬"°?xU7E)k?€$Â%­¥F?ï̜ý7‰ë?w¹|5É?I=l§Ú"?RUÝ))?v‰Ó®¶\Ù?t‡ƒ8›y?î¡¥#?'æÃÎ3o½?f'°Ø`ºç?sZ×(?ŸW·¿D=?'XmŽÕ™›?ïÈ*[{Ú?f…E§¼‹y?7‰¥¦7'Œ?'Ùlmá°?zyЃÂ?fqX"äü‹?ïk2Ív"°?'Þ'XBóV?f1ûŠz?eÏÁçžÓ?¦Íؽ%M?Ñ·ãÉ£?ïˆH{™ÔR?Ž§¼Ð­?S(4Í?aÇ%œª?‹ˆÚ¨¯@ˆ?ŒuEþò à?î+ק¸t?™Ašÿöø?p¤æ–,ë±?x¶]@=º?«-çyÈ?˜y]ì²U?ïøŽ‹bc?‹*ø+iH?YÇ%Í}Ït?Sójlñ 
?›"{ÑçѦ?‹ráLuIAGN4FGL J0220.1+1155¿çƒ×&(CýÀF´ê¿üÚ²À;Ñù®­'À<̹kÆøw@#£
VE1
?õS"¬¢ŠÚ?Øléã3¬?Ëv远Ž?ñÌI"®P
?üwŠ*ÍB¿ïSIˆà
ò¿ï웟-WQ?å
ë ¢wd?è7¢cl¶â¿Ç,>¼~K¿Ô''>[…bUNASNone?ïËò·–é?p­|^¥Õ?@Ú.ÝÍÄ?7$ˆ"\Ðà?wë^´F"??p0J͐
‰?ï¬ýÇkŽï?'¾(`Ž?VÆÁjÏôÎ?cX(1Íå?çµ÷Y–?"a¥F«ø?íᖚ$³?ŸÝåz¢ñM?gíô›?pÞΊBµÆ?°;Jé9=Y?ŸÐòU°Q?î¹ÜÍlÑ?Žª!Ìåh¨?6¨¤Ø°K?-•Hõˆ6?¤4áèuœP?Ž™×/â?ï›Ø;s|,?ƒîM¢m?NߋèjZç?U'‡¸F?‡øq$â6?'ÏIv?ïEÄÞýã?—;ˆ$"àZ?\g¦Rõ¦L?mvcïF©ò?•€éÁǂ'?•»ÙI,ж?íT֏=†?¡Ç&ј<?h2‡¨?sÈüο5 ?´"âsfÏÏ?¡…eó|¥?ì[6ˆŽj£?«=pÖF÷?J›ƒ†EÝ?Q&&þB ?¼ñ³HõÆ?«>œläƒAGN4FGL J0222.7+5016?è%H‡Œ.À#þ½LýÕÀ:âÓº&×ÛÀ<}œ¸2@ –Æ*œ6@˜Ð`Ö­?È\[öu菿Ÿ.'Û+¬¤?Öì˜ú¸B|@L+Dý?ï÷ýÖÚî¿è!"hýð¿â"ëSÏ¿ãÿëþ@bF?'o¦ß…ꙿê7]>ÊkUNASNone?쀓ÉK
?³À·NPê?ba—Z?W´»JQ?»j–¦
ô?³"\6f?ëI<æÔúˆ?»uǜ%(ó?aòtÞm˜é?mn ÏÑg?"BPù?»& Ý]œ?íú¿<ý?™%72vhË?i'¶Ü©m?aŠõ'ɬ…?®»àÏ	ÔD?˜Äqj;?ï¤q@qÒ?hú°œA?>dU•"¡G?+ƒ+¥¬?…ð*Ò9ê?híí£ø?æð>7±?ÄT$¯â±;?ogý@K¡?c՜Û<¯?Ñà³ØùŘ?Ä;`­ƒ "?æØÄñÐ×?ÇPµÔQ•8?c™ãɚž?vZŝRf¢?Ò'BU T?Ç+t\40?êËóÐ`™ã?¬2šª7añ?vW¸bWo?k—ëÿ¢ùô?ÄrüÊ<?«×NCÊÿ?î½ó˜ƒ?ŠSþO"Ë€?V{¢Ùû[Æ?O+L¹ýH?£{c¬*sz?Šy¸"
ØYAGN4FGL J0224.8+2937¿©Ã–­«õ<À<ÿÜ&Üã›À:¯Úv»œÀ<I½ò>v]@`+ŽÏ@.ȺïT·?DZ%fìÉ?ª;§\6?à‡f%ÎÆ¢@ajþüu?ÀvD?u
ï¿ëŽèe¯‡B¿âsՅ2à¿êcA¹óê¿å•€¸Í¿ðUNASNone?ïs>?¼ë?»Þl:?aÞ@*{j?Žh€Â¿?ŽÀà]âÚ?·¨ÃÃÄ?w¶4?'±û2aaO?Xý_«{L?`_¤¶DSy?"sÏô26?€?	?ð·?ï+nk¦?‡
¦gÐw;?hËIñ	õÒ?eõNÃt¯?—xÉaÕªc?…ý~FX?ïŽ65_÷ü?d,Ñ¬§?YU5êÝ(ò?>èzNHž¢?‰GËàW‡ë?bÆõU(¼½?ïsI;gþ?‹òÝä1?V]Ÿ³Þ)?Qf#—×#?0þ§Dºá?Šãp…×£s?îÂҞ%£?ª™CpѼ?k\s	–8‡?w»-nŸYE?¢)¨YïÃ?©¾QÆ'¸?íüNG`¼®?œGîËf?{§*úF,?uÖKÌU)?¬Æ6.àõ?šƒ'Ü1_?î¯$u!·'?ƒ£`صö¶?qZ¸u	fæ?_bpmß­?¢âaœm­"?'ZÐöÈáAGN4FGL J0225.5-5530¿ÚÞ`Å´÷æÀLvi¾	»kÀ:e'Kí>\À;ÑöÌz—v@‡_/es@°yK!?º!ÿ¯"B¿²ìÈío/?÷t'òÜ+@òÎO§Þ¿èï!áQ>6¿èsшô¿â4¿Ÿè"'¿àJ½ÞYÿäÉGNΚ¿ïøHEéïUNASNone?ïÁ~õ?s[c·s?\«½..q™?U'Zd,ÖÊ?x
"c±?q'2Ÿ 7?ï¤ûKÇ?†–"GŠz?`ŽuÈ?k³G3ø"?'´ Îô?³Ó2=Ô?î$	µ"þ®?š†MÚ»?ô½LS¢?6áûÒ±?©B5Q
Á?—¶o–¥nE?ìäd"V?"U}Ϩ?pÉr`(äm?Yúà4ùPø?·ÐHÒ ¯	?"fžD¤Ù?ïWa˜÷2?ˆÒ(Œ¤?x‡TMŽ™?l]RW™üŒ?úÝôjà?…qBŽAã?ï#$­^r|?›ÿŠ~?nžTåÅ¢"?NîýJ?—ÇŸ±ùœ@?—csh†Þ?쪳ó7?¦'jYäB¢?'¼aU݉?Šû3Jç?ºË'þÍ?¤Kç«û²?ç#¥²¾?­:¿»­?Œ\õٞ\ñ?€Ê'´*'?Ñþ
Μ?­)Bî$&AGN4FGL J0226.9+7744¿ç€­Óž‰T@/©	¾ºÀ;f6䘛mÀ<´ÍǞ@!Muþ‰Þ;?þJÃ")´?Ð_|½@?º}=msËÕ?ïÎùͶט@N‹•‰¿ë°ûœÄ?ïÐâ (z?èF4AÑ¿åá3÷~Q?¿ØáDŽ$p¿áò,}a¢UNASNone?ïÎ8iE`?jÛhaäY°?<3vyýV?+;í=s	?w »®a½¸?iýÉ)ä.Û?ï}oÏyX?"†º¢Öu?^+ÉÿbÏ?fD×
®?ŒùêÂJ°?"ódû¨?ïEÀ©}è8?'¿É;@E‡?dȪ£)â?a•ËÔ3Y?"®ÕƒC¹?ß|»'ù?îäÁ¦ËS?';מñH?k¯"»
#«?^Ö`EX? :¬Œ+?Z¿?û«x?ƆjE?™ÇÒÀo?Mñ{ª¤?AY¾X6Êå?ˆ÷6œŽ?":K"š?îÒ±
N'?¦x£ozD?p·Ûa¯¯E?à1!@ݍ? ½óëõ‡?¤Ú®äcÕ-?î¡{883V?'¥KÖ?o¤2Ñz?eð$´‡Â?£îL9uŠ?G°5ôT?í2KWIñn?Ÿ#´'ÌÙ~?wZŽý@€v?tJ¢pñÅV?´÷üVv[?žu´…n
AGN4FGL J0230.3+1713¿ï)±5±V"ÀCÉ\ú¬ÙèÀ:a"»ë$À<J›ñ@A€§…?š@ðHðŽ?ÈÿQ™Ð¡?șß9¶Úó?ü8­uïpf@QüïÕ:…¿åNµY+¿á†…‰A]¿æ@O±;`¿æAözE@|¿ïÿ"àT¾ô?ê&f%ÎÇUNASNone?î2
÷{?¡	àmÓ¨?¼9óQ«?w.¢F½±Ø?¨oJÐ-¶d?ŸÀYÕg?ïŸI˜?™tµtñ"?}™Êd
Uß?"erV¦Ù2?–ÖY…°Ã'?'WƒàÏ×ý?íÈæ˜ðI?›©‰+l‰?'EèÚg?ˆe+ØêË?ªâûôhÙD?—!\ë±?íl£b"èk?'t
H@Q"?ñ³)lCÎ?fÕâ€)d_?²\®‡¶nò?Mq'6A)?ë©¿vgª?±zBÇgí?–ÀÄç4´?sÿòõô?½ã¼ÊÀ?¯Ì€‰˜¾ª?íA`,\ø?³a0^§=?'#e\fr?žóáßdœ:?±j£§ñhf?­ä¨Z®u"?ë%ìJå(?©Á"9§N?£(*‡NG?•w;ú)f?½<ˆhçœ?¤ô"õâ_?èQès$•?«†¤èg?˜?'[¨´?†(Ví>à¥?Ë°kçžy?ªhÐíÑ|AGN4FGL J0230.4-1140¿ÕNlþ
ÀÀO"[t›À;ãeUÅ.sÀ<åycՒ@"Eñù31?öœªÆÇ©?ݎ½"à¥?ÔÐ&žzT?ù&Ui¾à{@õ•íg¡û¿ï.G P ¿ëÀãàd¯,?ï÷áî-¿ÛW
Ãbó?ʋ)¿A¿â(Ý9+š¸UNASNone?ï}®XºÎ•?¡íÌ«ýÜ?RG:§#·?rꅇ j¹?ŽK''õn4?Ÿ–ô	
*?ï̬ǧR?'0
¤ë§™?RïL£ü"Ú?cAé9Øÿa?xöÖvœÑ÷?}Ú4̵Û?î{kol?—ÃÒµìvæ?iôŽM±FÞ?qljoá˜?¦ª±…J?—J9r?ïoJc"{?u°>º'M?×ZÍÿ$|?
$	Uk?'Ü2ÆPÝ?u¥Ëßòƒh?îó8zYã? œ:Ö3?_Y–ä?X!öñl?Ÿ£kRÔü+? ?\kM!?LXâß?"-Üâ7¥Û?X¥Ÿ²Œ?n°YÕÿË?Œ'X*æ?'9ào˜ž…?í¥‰¥Á×7?Ÿã"Ÿ¯ˆ?iÃÒ3³E›?rqbߙfB?²"A$"]?Ÿx…šLu?îUv»ü¤?•·Gº?5èAim?!–Ñ6Ù´?ª¢
ØL?•MÃ(õrAGN4FGL J0231.0+3505?ìAdi¿"ÞÀ7wÂôÀ;¥`úÛ4À<ÓW,6¿°@!õ¸¢žP
?ÝáÓD59?æ¿qdÇ)ö?ïÿ¯Èe_@SÞ|!¹Ž@‰\N4–`?î`pî¤ü¿ì¶´ÝlØ¿êނ׶4Û?䗖ºÖ*¿Ô:睸0¿è'#ᆘ5UNASNone?ïHû¤{Ÿß?"xè˜1?pÍÓ*,¹?t£)ÃG?'­¤Z?'ŠÔÞ'ãÖ?ïa
T,?ž¨ÍnQO?lôý[Hšµ?|Á
&ã|?@EmïÞ?›Txϵåt?í¾x:F½?Ÿñ¯÷þ?'s´F‡è†?'H·àɲP?ªÞ£éŸô?šÿB
©‹±?íŽ/f'¯Ð? ê/<?aìD´ðw?iG'Ôq8?²ÿ U6È|? 
=½½?î9gw)úr?ªáhÉĹì?"`י?™×WO>¤?¤ˆpZé­?¥Û°¹r‡D?îp£Ñ"iY?²Î‡Ï:è?":#µºS"?žÆ¡ÜÖ|›?£ç:®v¦?¯9¢1Dzì?ìáTç
æ?¦6–ñÇΣ?'RÉ*'¤?'>dL•6?´ ¦|䩤?¤ßù搌8?êä^U~j?µæîúD?fmäþ}?wãOxǓ?ÄôæÙ?µ† bg}AGN4FGL J0235.3+5650?ÄPw¥¼
À	ŽØ'ãt¯À9­Ž»ð·À;§³Æk‰¼@Š^nJ`v@Ð >cé?Àã[š£~?×êÁªYÛ>@¦Ñµ(k@KªûìŸü¿ÓÌŸóOî¿ÀùÖZÀ¿çA>U¦%¿êœ}ÿà¿ìèÓ=ª/"¿ïÿæÀ
UNASNone3FGL J0235.7+5647?ÏÓ0Á5aX?»6ZZ?ÌG¿ùˆJ?½Fh¸-áî?àùo_´E—?ÂÓs‡-¨§?ØR³PÏÑ9?Ç܌=:ž?¼éњ£?³ÑAW†?à9…vTn?Å!oh»?߶\&¶<?²ÂÌäaÎX?ɱ쮋æu?«*Th<Hh?Óp­'ÐÅ?°†¸K5ˆx?ä"È	Õ§ù?žkñÚg-û?ÁªÄ±˜?'†ފ®R?̍Î-䮅?™5?vYr?½óÈ,¡k?°"L÷>5Q?Çí¾$úq‡?½¤H^¾|R?æF.ý»Ïq?Á#¨z£W?Ä8°–?¿îššþüþ?Áÿ·ÁÞîI?»ã˜Z>)?æyCìF˜H?Ã^H·Ì,
?ÓÉ81Ž‡?°T¨g¬{b?Ðe–\Î7?±¥0PYÿ?ÜÃÑ1q£B?´j@sÍ'?×±Xq?£øA=ÄÛ?ÏõƑÛpe?§*S<r_?Øïòï\?¨FٗO@MIXED4FGL J0237.8+5238?êyHL¹°ÕÀ®–ÃüC³À9ÅÛ_6Ç<À<VÁ1Ž…@Vá:B.?üèM&#€8?¾ÎG*`ý?㎧Þ*î@ tNrSÚs@T	|€"¿©q¬]f–¿Î÷çؖڿˮ)7'¿ã®T§!A™¿ïÓ4*…¿ïÛgNnUNASNone3FGL J0238.0+5237?YVdcøe?'ÿ¦xV&H?ï9íȬ?šêÚR<%?‹¾×ÒËz£?ˆaÛÎX¤B? gæ]ƒf?¥V-«û??æ^œ£?ÁJR/ëÖ?Ñ6Ûû$4N?Àƒ§þõ3?¨p€C!áÔ?
Rbz'÷?ìªD!£®?¤¨n¿Ùt?¬ë>>3O?—î+CŽ?Å™Úå? iœ'!Ÿ?æG5¶u?¦¯Ål:£°?ÁÞ$KCî?›Xßð4Ô?'E#O*T¦?~_Ä×Mß?ï6äi\Ì?''&fNÇ?á0Äßg?ˆ Eç2,?ú­ú‡l²?–1ȉx¢?ç8·þ£Mf?Æ=ݸNÞ?Ð~å"Ùô©?ŶÓö%¥p?"[÷(">~?ŒÍŽçڇZ?íÀËÌãQ?›
ò|¡Ëž?©ÅRʜ(½?"cå·è)Ä?¯d¿'êY?'UÄërxo?è¸u¾P¼?©Ÿ¼ý¯•E?ÅFºFç¹?¤¾¯EÛßîPSR4FGL J0238.1-2621¿ìՏÂ2ó{ÀPŒ¢3œ¿À;쪸¥ÎÀ<°䭔"@"³Ä=1@"Ã9¦?ċšþôg¿Š·t˜O¹ô?Ãþ$@­š@
93Ù?ڋւ®°¿ê3*š}£¿ã›¸øÚqÑ¿ç¼àáVǍ¿ãÁ2d×.¿ìÚ¡oBUNASNone?ïû+0Ÿ?4N¢¶fÌJ?¬iŸSmD?7
ɕV?@}°"²É?3BávÜ?ïßü'|?q›È-5Ú6?<"ο|?Iéå&?mg€"H|³?nïêUî!ó?狀ڏ‹¬?tUø"4®?R©ÍT@Më?L‰á€u?ƒ¼´¬±+?s¾½8±×'?ïíqÈù?B$þ
çé?$uTmq<
?-O\Ô?a¶
M'µ?A¤$R;×]?ïð-žŽ?T­ªðÉt/?) ¨.ú–?áÞîÓ?\p®H'<ñ?SڗhÏeÆ?ï¦Ï…f1?‰¨÷¹8o?LuÏeŽ%?_D¥ÚM?""â˜àû?‡jÀŒNaË?ïOeq°Ì?"i=]
	?`ÇŠ¦Hì?[pÔµkµš?"ún#»h?"%ÀBø‡?ïÄtñïq?cËï^r~.?>>ǶZÜg?1Õ¥%:?{ᚠ½?c4Ϧ­¨AGN4FGL J0239.1+6634?Ă9ô¡Ð@¦¨¸ñM¶À:!¦+xSÏÀ;¦åßÃI–@K|¯Óí¨@îOá¿£?ËV¢ùê'0?Ì2#(N'Ö@¢]<ñøÖ?ñ
4EHß¿ïþ] o!?ïþ¿Þ§À¤¿çËxÎø¿ã#9 µ—§¿ì¼¦¿Fý@¿ïï–áXuUNASNone?قtóá¨k?Ä£$ƒ~5v?¤±+«†Tc?¡ä7fbya?áó²Êö'u?ÅyŠ£?Ó¡;UÁ?ÁçԓHO?Ç=テ!Í?¼±ÙÓÔ¢?à_õ…Êý?Á	)x¹ ?ä:üžÝ·g?±Èk²3L?°*-6h?›oã¬|2?Ó"öÛzK?°V˜¼²Ÿæ?Üúj`V5?¤¶ÔîÓ^—?ÉJ‡œ¹V? þ•›Øð?Ö`†žÑM ?¤okåå?ÐOdáDíµ?À›ž±€Á?²¯µæ‡½?°$™Ü°P²?å'VÒ¨6ž?÷-yñï­?¿wW<ì‰?¶%@ni›ù?ϐiI'?Äa횼?äi+úÒ%?ÄCÿ`jEf?Úª:u5¥î?²»[7€—7?½RkßR?¥bË˦)?Þ*Çÿ³?²"sZ Ð?Îq±N¨?á?¥¬º~X¯ö?Ñ	÷î—*‡?­Ä–øs|v?ß½/jµˆ?°/¡¦½MIXED4FGL J0240.2-0248?ÈùMØ¿¹ÀK1ÿ`Ï‰À:Ïú÷''ýÀ<{q°F"I@ýw:Ê@g&Š®D?¦‡h¿‡¿‡*[?¹ ?Ã@ŸØMœ@òïÌ+<?ãº4¿O`»¿ê{ù?ò^W¿çAÿI ÛB¿ç1‡+ØË߿ҟhûìõâ¿ïþú·ŠñUNASNone3FGL J0240.0-0253?ï̅+ùX?‰"Á	8ý'?Eœôßrf?R".éaÊ?w	ËK¾}}?‡wøÎÍì?ï×Ë¿—Á9?q¹Š–?ž±?@Á7šä5¿?IͬY¶?rùTj:†?o!€x¡TŒ?ïX >_?‡X]z‰§í?WJj' ä?Lö¸þPDy?"Š…T"*??‡î	4?ï㐛n0	?Iì
ÅR¥1?+:±¿fé?IÜûÌ?j½à®}—¶?Itú,?ïeË°w×?'àÍkËX˜?YÕJ¸£?U÷‰E?'µÁ81.R?'Êτ~?ï"ÅÄðµ_?‰ÁŹ†i©?M$ãȒ"•?[Žm^ìä?ˆü@qØ?ˆV°ô{©?î™Ì++Ç?–CÞE'ùÚ?dJ°¨Sñš?`~Œ T÷?¥'@£¢÷?•Ñy•"(?零`(Îo?j±€â±Å?Ež7‰Ð?:
þY Á?"ù"uL³?iÕzä)b2AGN4FGL J0245.0+4755¿ì(;þˆÜˆÀ%vbwÄ\¼À;õ5¾À<X;ãv@1ˆc;d@+­Ûoý¿?Ƈ%£¨'.¿˜Q§E1k?ËƟ¡›p´@ˆH®ðn¿ð?ïÿÿ^ðP`¿åMv«Xÿ¿é'öè)J¿Û­"\›Œ¿á2ÚþhÑ%UNASNone3FGL J0244.4+4745?îJfž±?´*mŸ$Nè?câúhíÑi?vè"ZŸ; ?ªfxZ×?³Â±Fo·.?ï_åŒûë7?Ÿ¢Ëîì·m?C,í±ñ~?R3CÝ[-?"iæùsÉÑ?ŸQŒk‡U?îçjÃÿZ?™z"+Xƒ?ƒù´ÐՏ?†<ªæéœ?©3Ai	Œy?–?¤?iŒX
?dK!8Í?Ndt͞?8!$Ð( û?†5ä²Tx?cž¼2´½?íqäSÒ?¶-¬gȩ̀?r'à}Ø"?sô	"ê‡1?¶;Yrb,?µÎ·-ø7"?î±'Õ™
?¸¢rGzzá?X2Pzbçí?zîDŒ¼?­"UK¥´Ÿ?¸€"cHï?ìY'tÊ?¤¨¸¶rè?ŒPÇa¶¥Ú?‡õ¹èßöø?»ÝäLERð?£-ǶÓà>?îæÜ·•Fè?'Ðxù±?cÛ|¾›Ÿl?Wß'"ÚÈ? T|·"4?'G	'"¼9AGN4FGL J0246.0-4838?ãåêmFª^ÀM£~õ©eÀ;(×å.ÃbÀ<h¨-±@ç×õÊÇå@µî;²]¶?Äç©Ý^•b¿ºHY`™?òI²Çh	@ˆú:U¿çO¶@ï3¿éG¿å‹<¨&û¿åJæþ§:l¿ïÿýF\I?ïÑ6‰)	UNASNone?ïØ´m=	?€54og?\«1yÑ#ˆ?cþŽàxÃ?höJ"ÔÝ?{²ª¼™¢?ïµ¾'(d?'¶"L½æ²?[Í1
£?g8ºêøµø?~-k
ùwâ?}ä>T`Â?î¾ÈvÀ•v?–)Œ(]ec?tE¤¨?x§—Q¡?¡ŠÆh_²?•rÊ&?ï¸ÔUéQÏ?f†`Ÿh?Jù¢Ñ¾¡ô?;øᐁ?€PQá˜?e(­±É"3?ï}
bFϦ?"N]•ŽEs?€ªÄ4Ýã7?‡`w"ÁŒ?€ã?E‰N?‰š;åeHO?ïSðBë?˜dˆÝã	J?g«ž@ªºˆ?zÐìÞtô?'©È¸VxQ?"€R%Ôù?íÃîkFä°?¢æ·ß/?w[œCÒ«?y$Ú"mû?°jÒß²îÚ?¡®yÍ3k?î×/êSpj?²M`?mP™d ;?f8d2ÍY? ·÷È`òØ?=û¹o,AGN4FGL J0251.1-1830?åcy­H«žÀN—ñ{ؾsÀ:öbWãì¤À<pD5¹ö0@!vfóT ?ôç"øoé?Ñ8՟eæ?Ü_õ~F×Ö@Ò¯dÜùk@7µ	Œ›¯?ï0ÒÐòÌ;¿î×Û'Ùc?éätSŽóM?•Q:]³¿Ñƒ˜{au;¿ãáý`"iUNASNone3FGL J0251.1-1829?î÷ª'ŸÍ?–ÊSëÕ?"ƒòwÞQ?ÿÔαMõ?–ÈÃl•™I?'+@-i0?ïœCt–LU?'c".bÂW?bßÇY¨c?n¾ˆ6Pç'?"71É:¯?Βa`?ì£ð×\âs?¥Šç½"'?¥©"‰U?›Í€Ñ̐è?°빪Ž½?œBçþxã¹?ìG=Îý? bHPz¢?gf®æŒÖ?VÁä–ö…?½8¦^õ? P‡iϨ?M:?¨jEãÌß?nšüëÚv?-dÃø2™?§Ošô(?£þÅ{jš?ï.)«lw?¡m üÁ/€?tW›ïsŽ˜?†Lq~ºžŒ?˜$SÓYk?ž<î²u"Ÿ?êpêLJ'?¬ÇrÝҊz?°*ðt9?£Ÿ"AYÑ?¼Nœ°¥NÚ?¥¿ðyý?è'
M	b?µ¶•ˆï§?q·'ÑÇéÿ?oÀÁôP"C?Ïoû4-?µÉ°ðo¶"AGN4FGL J0251.6+0628?Áÿ\þGÀFÉD€bïÀ: ­‹¾åƒÀ<'¤ˆ
%@2au»Ä@ZYÀe¶=?ÄûZiXU?¨«œÀ.rž?á—ÈAíá@ópOžN¿ïn'>´Ï?ì'VÃ[4¿í?Í«Þ¿Ú4çhY…­¿ì_Ïsp:?ѝV}JKUNASNone?ïö"ͱ?¢•€Ùyñm?jCÿÒgOG?pF°.¬?˜ø­›òñ?¡N]VÙfÊ?ïÇSd'7?x^]Y}™ç?Nþæ?Xÿ³ö-kŽ?x•mw–&U?sñ76ŒQÝ?íG¾i¡s?¥%Ûæ()?¦ÉOÍê?®jÞބ?³3'1S%?¤¤Ýt®¶^?ïÄâ{=l?iÙj3·R?_ª¿ÎŽ?FDG*Çr?"œÃ'÷=?fß+›ýˆ•?î
)z%-?®Dç-?nލ•?}œ¸H"è?«?­ÜE†?¬ÎØÚfV?ïSªè݊Æ?•W_dô£?av<6'ï?q˜į?"i"PXÞ?'æÊ8˜®Õ?ëµyGzÏ?®'Åc
·?Š-+‡BT
?…½Ÿ+ Å?¿Ufþ?­¡Åònñ?îôSÎMR?†š¡ˆN¹9?wr| —Á$?h… _{ы?›˜ç?w?"<úvÇIAGN4FGL J0252.0-3657¿ï!ÁÞÝ£ÀO`˜²é̸À;ŒôNÀ<꬇²çH@ :¬þT?÷ó朁«f?áHÌ!¬"?ÒMÝC¢•?ò+Z;µ¸´@jOøË¿ïüùOâ–c?ïÈNòÄ®¿èEr/ÈD¨?'{o"i©¿æ~râÅB¿ïëá/Z`ŸUNASNone?ïò%YUÜ«?PhìÕ59
?.¥aΜ"?$üXm	ܸ?Wà›6ØÔJ?MˆÔ57ÖI?ïë±*e.?gÔ)0ÿ'ú?.†ÿ×hÚ??
Z𢷱?bf¾*xr?eU)û'?ï+Êddc?ý"\U?eÓÏ?qëQÁïq8?—Ì;°+(?ŽÄÛ¨?ïËs'ý?[¸é88æ±?4F@ð1{Á?&-@SÇf?yÚÙ©vÖ?[4?³+^{?ïå£+eM?aŠ"F5Dä?<fxñ­ËÜ?5IT
ë?fÐr£ø?`#,¨,(?ïº@'Y؆?…‡—Úì£?Gm³'ä%³?au­£O?ò5ÔX k?'é=.&^…?îó62cvê?'
mŽ¿D%?eü•›ž?n×xø'X?žàÂ)$:? Ô֙oÌ?öB€È?t£°O¼Ì?4€7ÿ¬Qª?87Da]žH?‰2º,d¢?sÜæù[d—AGN4FGL J0252.3-2707?ï÷72W|OÀO•[0HÀ:Þ\î 0À<¤¯¸k@…kûü4@x¦f0·?ļÚçB¿¨DŸ[f?Û$[)'=@æ"B€¿Ãø*ÞûÎm¿êWådsG¿ëˆ{¯£Ç¿ãýBJþ+¿àvžÝ¦8ä¿ïÿÒkÀUNASNone?ïùªÎ 6—?I#®…Ø?2ÞI˄k¥?68ÁÒ??Ë?Øn@<?Aaò$ô?ïåúl‡ª?p(¥éóŸ?8ý£t…Ù3?O—"n'Ë?fåß$‹£(?kVW·×?ï(k½yƒá?-¬ÜM…?nñy­%Ÿš?{plZ	vw?—Y^¬õ?ŽdKÌ4¶?ïù×ڜï?0d²§Ü0á?"SZ<ÿ?QT|PÇ?DÐ0íˆä?-²¤‹?ïó"›t~ò?W˜'¥?D?þÝ)xz?E‡ñe¨‡‰?M­"éÕÞ?P'ƒ[cì?ï²'úæ]?ˆ½½Ÿº`?MÇ)+;ÒÈ?fŒ"CÚ<ý?œ¨¦' œ?…5B]ñÃi?î‹ÍôȜð?˜3Õ^y…?sû8‡fT?~ùbIþ©!?¤âHq·<?—›ØPH?ïìcf4oý?Rǝ$sëË?<ž†úÃȝ?644ícYÖ?`ÉBMç?PUò§0AGN4FGL J0256.2-0408?ÀS¬dÀJ2ýX…ÓÀ;Wy{ ÔÀ<²°9ï@ »Ûۈ?ÿª÷	º?Ó÷e<DÔÆ?¯i³í'Ð?܆p|¿Ä&@GBW=?ïضDË,¿æ
¨ÐnB¿ålKîñ¿Ôè™Fƒ¿ÞZZT	l¿î.R¬,ÄUNASNone?ïòÎC'ê?NR
§ž³?ì?(WN?#Äõ'Ræ?X…º×%o?M8¨Àÿٕ?ïÎín-E?s¦*'ÿ´?Bç¿$—0Ø?I_j2º?v,QسE?qÐVAo©ä?àB0¸?wý'VM@Z?RräO?H««â,X?ˆDú˜Óo?w–j÷Úìo?ïÀ×Í ¡?\GÑ4v†?3!"*èF?p-qUe?~bÞÊÀ?\JM¹kÑ?ïäýÙgÃf?[‹ý@\bi?*ššÔaև?ÿ?¯'íÃ?iX|Ç:Œz?Z¹#¸4ó?ï‡ÍoÆÁ?ŠêöAÃÍ?NÁL,
Qÿ?]KŒÿ3?Œ H†!Z?‰V1®Üst?ï9'½µÕ?‡+èãší?XM¥"K?OC:œy?—J×ç‹?†¿.9à\³?ïCXšÜ÷?zÙº?Ý2Ç?C€u¾·¨?8HÒDßà?—1I	o|?zÛñ%K×AGN4FGL J0257.8+7044?ܶ–f֛$@$ËYWŠ*'À:6ÄÂ<PÀ;Áœ¸2@»	sq@N`›KJ?Ä̎c…‹p?°ˆ›ÅmÝÔ?ç?	ËZÜÅ@~Ñ{]A?ïï;At"|¿ár%acr@¿æ,æ³'à¿è¬ôŸú†Ä¿çrSÚr§½¿â€fWLíïUNASNone?ë¢wí*?ºz¼8äí?qýÐ×D´3?e›¼7Ó?Ãm‡š
$>?ºTb©~¥3?ëI"óE1?º*¬üÍÆr?'5±|)ë?Z"—6æ?À³›àVþ?¸€×$ƒ[Ù?êãe¬~C?¨Ö"î+o¯?•RîôÑ?‰Å‰¹k‹?Áȁa?§øU_Û?ìiÄâ?Œ†— |ÿ?"³3)ÀF@?pn=Z1"q?ºâ?æP?‰·GÅ+)?èÖx´p
?¿ÿ3&s]?'‹H@‰#ª?Š*k*ÉÁÐ?Ë}ho™Ú¡?¿o¢WáÆã?䙵ýÂ&ð?É÷¬žìr?¢¢<¢ÀX?§ÎIGÉM?ÔxLp#²?ÉF‹ÆƒmÄ?å²ýd€n?²ë^âëE~?¨0.ÌEj?˜ Ðªñ˜?ѕØ,Zµ?±°ÛÓÆ~9?å›Â©»Ù=?¡Y,yØ•?©wá
¹Œ?8C4Õl%?љ—ÑB}S? žÐyÐ]AGN4FGL J0259.0+0552?ÜàvG"ùÏÀFiÕ^kÆ"À9Ìü}"€UÀ;êêÏS)@˜{RÜ8?ýì}6Œ"?º–R<bÜÄ?ÁÔDe_«6@Xî¼
ݪ@	(±‡w@¿ï¶öÁèÃ"?ëX½0w—¿Ý{>ÊÁ¿ØV«ùµä¿ä÷9½ï§¿ì×B4ÍgUNASNone3FGL J0258.9+0552?ï÷ëYf	?B¤÷u¡?1ȍ,í‰d?*õoÀn¦?J¨PèVÑ?=ìt2Á?ïËü
4Ïs?zYûì#â?KsÒQ¢?VÁ©	!‡|?v"~þ/ì½?v…Z˜»?ïœ)«Â]€?~åÛÛkG¸?bo$'3?j«'aºÌ?"YÌóÑ?zQÌò¨¦Â?îØÏSO?yÎÝv§Ìï?q6fԀan?Q_S>マ? LAVtqe?xâ;®µÀ?ïìK=s±†?Uôܜ[?M¢¯¼l·Ä?FÒð"X~7?X˜-˜õpä?LÑ\_0n?ïg¼# /d?'hù` ¤?_dMù' ?t‰*Dyè?'6Áæa?½Ëƒõ¹?ïPcÞÝם?‹{³YÓß?qða>ð¾â?xQa,L{?'wkѝ1£?† 8@σ)?í³ 
ÏC?'–OØÈh?€?‰ÒÚŒ?i8¾­5š?°[
Û1Ú?2¸žsq\AGN4FGL J0300.0-5908?è2}(ØÀIˆõn¬†À;¶,c5Y~À=™'óe@ 8ÅßÉ?÷Ũ›•\?ãp"'0Fo?ÛÀ?øzDàÑ@hÀà?áÒ¹Ág‰¿çâ,Rƒ[¿âü»§á[¿Ì!ðj¶­&¿àÏà}ƒ¹^¿ïÿ‡4<G¯UNASNone?ïËðí¤™ä?pêæŽ=?QâÎÌYó?K
å ¼*?uŽÕKßh?lZ¿Þ¹Ÿ?ï¹'‹V­-?}kÇÿ©ˆ?S*åô:‹?]ÿv!mW?~¡€÷>îÜ?x4"=•˜?ï9ތ׃?˜î>…£x?tQ®!/_?x6;§Q7]?—d'»¥•Î?ŠÊKßLb?ï™6-A>?fán›ÇL×?E_S颼	?7lï:¶h?ˆ\n}T?fZéJÓÙ?ïšccÛ$\?€Ë§*HJi?gmÞʺµ?dë_6Ċ?ƒ‹¯O©*š?|0¸CM¾—?ïMŸHbÍÞ?•j՞Èý?a‡÷NÉn?yi¢¹.‡?"5Tdu?'폭5?…2s?"QšºF†y?w×H§]ñ?~€¼T¹Ó'?¢tž(?'vl('˜?ïÐ
¸¿?…
-Ÿ|Zå?H8V×R ?N}? _y?Ÿ9dizÝ?"Þ³ü‡ª£AGN4FGL J0300.4+3450?ïԌKt¿èÀ4ìûTŸ"…À:Þ½Ÿ¤vÀ<X®^L¼@pâ²gEß@—XA	µ‹?Ѻˆ¼ývä?Ïg¼&âAÿ?ö	Ã}˜²@…¼:…@?ïæ|Öë3À¿æeÔp/=¿Þ*t]J¿é\#ý`='¿ïÿü¥¬¨?ïH±(UNASNone?ï|a{;æ?ƒOúfÕve?g՘ÈL´?_ŧ;..†?Šò:ìüGX?'é5à¢ó?ï:ÍÓ è?•"ÈŽA?{"Ð$JØ?ƒ÷Û+§Ô?'Á—Q÷·?¼?î'KÍ?˜Ò È¡?–ÕG£5WX?Úƒì¦Ó?¢œG|s÷|?'Ö|™›¬u?íú¤—µ¤ù?‹
ÐV‹?Š££Ÿ4?p55eÃKj?©¬Í›,Un?‡˜i<t?ïdç
eµ?'Œë´+f?yQÚ+'"?rЉÂü\d?—>ûŸecò?Žm"WÌí?í«È%Eá?°=ìî*?"Æ\$«÷c?¡%uuù?ªàO˜f
B?§É±Ú%O?ì⿓å`Ô?¡È;H¤‹D? û&Îü?–½=`ÿ6f?°lpX½d?™ÄRxõiŒ?é²Ü»yµ›?¥0
ÀÀ}s? ;ȉgö?m‡®9Ø¢?Å%šñTãÔ?¤õrƬAGN4FGL J0301.6-5617¿ïà
½PáxÀJZæ[ê¢À;ŒAÀ<ÐRì6 @ 4±âe»F?û˜ç<º›r?ȗ…4²º?ÊU»Gi@½&fœL@ŸØRg?éÏYoØ¿èBã_5o£¿ÑÈ¡jÉM¿ä9[€Ú0
?£¢y^ˆ	¿ïÿÿÊPËUNASNone?ïÖ±íÎO.?ŸºcÿÞæã?HöÓù+³Ò?HòÏj­j?qˆ.µ¼9?Ÿ··GŸ ?ﰛáøþ?"2$ÉB¾"?T•ñéÒ{?`~¶€?FI‡ÕÄ:?ž©vÏö¾?´Ê^?Ží3x.ˆ?jMø¤ —'?siÀo
­Q?š"o	ÏK?5
-.@?ï—"©M@Ð?jüJ\{F?<ì–+jsI?-›züɒ)?‰Oðïq‰?i¬¬«oî?ï¦úfý©Ó?<ß\ƒýé?b°¨"w9ú?^Úס™ò ?•<)1jÇ?{¿;š'ô!?ïECìhô`?©»wPH·?^£-´§ý?m,r‡?•mO•'Ä€?œW'|ã­?îCí²0Ð?—pg«Ë?tc[dj»È?yÒR?²"?©;•»ë2{?–JDÕnG?î¥uÜ-Æ?‹Wq
ÛÌ?Rü§9ü	?K¼vù Aj?¥8À´è4?‹J¾q²AGN4FGL J0302.5+3354?á½ñ×bÀ5…aܓêÀ;!?8$4À<çÈі@!î>tÎ?ýìEz]"?Ë
¯–:|?˜P|Å"‰m?Ðå³£†Œ@9°â‹{?é ð‹C¿ïÔJ«þ?í]@þ"b¿Ý¨áá¿ÝÂ)ÜÓ¿ÔñÌËö
8UNASNone?ïׂÝ.]¥?i&þ;˜©"?$ôH8ÁN'?F(Æ?s–ï.BPç?hË23}Æ?ïÀ[š…|×?€€DlÄ4?N<Ȉ®2?Z™õüÏ}?|
™³.8ø?}²oi{ü?ï#³¦vª?œw*ÀL?Q"ôb­?S]‹ kâ?šqP¬9†? Žiü?ï1xÏäH-?|¥\JG?HŽŒn8…?:}®BÃØ?™qŸÌÛÞ?{ë"h'í?ïž"Œ¿8?~håkÜ÷W?5=åVò?)'‹'ú|?‡Î"#î.¸?~z›?ïd'¤=?.?•þ­Ö£¡?XÛ»çõ	¾?oL.+Šf?'áï»è˜?"gî´z±Ò?îe}<Ž1?—»2É~ã?TOUó8†®?SÆ?©±ƒÛ¿?—´ò¸Bú?í¥w?šÓ&£"?Z\ÜÊ?VžÂµ‰³?²mÞº©íK?šÊD_¿þêAGN4FGL J0302.7+5717¿Åø–$οòÅ
 ÒrÿÀ9¦é#D¨¦À;@«‡ça@'î
_)†@Gá%Ie¥?Æb Â2À?±Ô9}¥Z?çˆÜä.?ýE´ÒÛÇ?îïsàøRâ¿Ø\&$p¿è¾ne8¿é 6Ff—¿ïç"=ç¿ïÿÚÁ,/´UNASNone?ê¯Rc•?·×.;nïa?ƒ±[Á?}è7øB?Äœ¬ëÓE?·]¸{ÎD?äߥÂqÕ?Æ\y2pë{?üˆ+|r?SŸ)õs"?ÖÄx1Œao?Åù¨Ã-;Í?å|.¡þíÜ?°F4ë	Ç×?©šŠä­»¦?˜AzTÍQ?ÑÔQ_‡é³?®€ösŠ?ç JbÏ­þ?©tAñ<Þ?§½ç¼ô.ê?†N¿äX›?͏\…MB?¨'â2ï?æ.bS‡;ž?Á|ƒ@%?–¹aûí?'WƉ"q?ÒCžSE?ÁPÝÄ}G?ÕgÌ¡ß?ȚØY¯ ? ´àòɋ¥?°Š"uy=?ä@Ë  V?ÉW˖Êdñ?Ýûèñƒ?²Ž|¾è?µƒ¾Ë^6? y¶'ç7?ÜÀ÷w˜Ï?²b»åE'?ß^ö§Þù?³1ÐÿÙ·?¶Ã™´
ç‰?ž@ÌߜQ?Úð"ëp§?´Ì¯"jMIXED4FGL J0304.6+6554¿äh=*Ì(@Ü ~$É
À;CY7©ºyÀ<Ç
GžÑ@Üv¸îô?þc\ƪt?Ô|_p#?èç~>tYï@
‹(Øf^@Ê.¸Ð¿ïüÿÐ/WÜ?ïtÿ†]?Û‡!F÷‹¿àÓöAC/¿í«ŽÄS‡¿ïò 
¼%UNASNone?了`y3ë?Àuqt?³ËNªTtC?¥¹¾º%ÛP?ј"x{?¾¹ôOj?Òy5G×Ò\?ÄÅÁÀª)µ?ÌîœU`¯˜?ÁÌ+½,a?ß|wÕØ?ĉä¤é?éUNa¢?¬»+*IVk?²nHÝêV?žVۅ¬±?Á§r
€Ú?¦›IàÞLˆ?æÀú±Œ?§†¢ÍÉ?ÇEîMóJ\?¤PåÓ\r˜?½fŽK?™âïù͋ä?à\C—{Ԅ?Âz°GA;?À¾ÎÐe¼%?°Þ8ŒNÝ}?ÖèhÕxå?ÂZÛo›ï?ÅéÉÈ5ŽW?Â!?ÉLBV?ÐÚÚQDÁ%?Ç~Ä´­ú­?â eP;Ø?ÉaW'iþ?å?Ø»¡	?´(:'?¹ÞÍñ(Í?¥`±½õ?λš˜çv?²ÿ'0"~?ßvÒñ:Pš?´à»€Äíx?Ò5ó?µT`5$?ÍUý"òæ?®@ŠÏEZÐMIXED4FGL J0308.9-4702?ßEÉWKìÀLDõýG¾ÛÀ<U¾š#À=,jËOõ@"ókò¬?³‰–íï0?ì(ót'Ý?ïÿo¾ÁÇ@FÍ)Á@,xËëÚ¿ïûÁa´¥å?éßð•ÿ±?ï--àôË¿ÚJ
Dý`?Þæ3:¿ïo¿ïÿñò÷UNASNone?î0"€ÐÊÞ?»|¤Ö¹Š¦?'ZW~,?©ù8{÷')?¤Iœoü	?µ¥){?ïÌ
{#óá?'i!×?O''œ5?e}Èø®?vaþ¼g?|ç"†7ž?ì˜-À}N?¦}ORvåþ?£DÆŠ(?œ—W+'N?±œ.û§<?¡õPjúÀh?ïPÛÝql?…QÍ1‰€k?I	ã?dª;'?•Û<¶›†N?…P¼çύ?íëüXç³ê?´,…Í'x?—u
"^/F?¢t€¥D?¥…³±é^¸?¯Ëðâ^b?ïiµèÒm?¡ççÏ?jd?aHF¹c?'áËNTò*? :ƒZ­?Ÿ[]Š#ù½?ë|&þDó?«Z|å)Ñ?¥»ƒ˜39ª?¡K¬&¿%}?¹Aªa?¦8ùˆÑý?îõ`9_?–<åÀaû
>îǀZ¥r?+KsÇ´d? ­iÓTç"?–<Qd؎ûAGN4FGL J0309.9-6941¿Ä2¤ÀǹpÀE}Þ?»×²À;S'¢xæÀ<ºôúé?Ê@u~5ºø?øÎrýMž?Ûh«î/ô?îº@ãÉ@Û¼¾aÐ?øì–ց?ï£^>y¸S¿éŒþ–Ž¿ØWæ'öÀ¿éÍΟµ½g¿ï`Ÿ¨žð¿îs´ÈUNASNone?îKVët-?¤CO"#p?VûBU¸âÁ?YV­
5 7?§3p{ÛF!?£ö€¾@õ?ëU"?ß­¿?ÃÎrý(?²¨""ˆN?º9rÝÜÙ?²®YnÄw?³q«Ë|?ìæ»b"?£ÛéwÛ?š÷‡'YT?'ÃÚwê¤!?²FêêÖ? h$¡\÷÷?èF&ëQGE?«ðS
éٕ?°ú!ׇ?›ê$,ò?ÆÜXÕrýg?¨'smžö?ëB)æáÔy?½¦Ž/ê:?tÈ0KÈc…?u™Y¸mF?ÂQâ´Y}?¼É »{?æ–0+ýðí?ÍÂ	€Ãp?ÀÉӈ¨°Ž?Ä£Ýë-5?ÄÝkÇ_‹½?Ân"n%2Ñ?ëdú «˜?ª¡SX^ê? K¬K®òJ?"ŒÖ£Ì^¤?¼²Xúu ?¦û¶M½Å?âÝø ¾?º	VQ+§à?±S´'zbÞ?¦Ö'ž¤r?Õñê˜S?¹š_^¬«AGN4FGL J0311.3+2940?ÝL^Ò73¸À8}E¥ü~À:"å~tz%À<EuU³@Ê®ž8¾@µ¼D¿L²?Ò³A Ùß?â-Ánʸö@	m‰‹.œË@´0©kۿك#€¸¢¿à(ýOK˜¿é3eÞPÞ¿íšÿZc¿ïø`ˆ"?îÜÔ·|ÙoUNASNone?ïOøÓæÇu?"Lä	Tg‹?‡.Ø«}G?Œ À¦	$Ó?"Ó¾4Ý}?ƒTò†Ø'?íêÊ;ÅJ?®Æ¯k+áÊ?'•d?k?¤!qàZ,Î?¢–¡•'Ÿ?¡Œ²uE—Þ?ì2xKé(?¥F¸ð"Ǔ?£g=З?•lTK©ž?´¸¯LÌù? ³¤gõ?ë<­Gˆf? ô+Ås™?­ƒ/Ã鮘?Të."Ç?·Xÿڅ?™ó¼9|"}?í¤M|é?­ÍxŽõ
?§Y5wòZ?¦KCýA?Lƒâ]?N"ïeÈ?è/ê)M?Ƴ•¢$i?À§ê·ÇÛ?ÁÒC³wÕé?½0Ùç'uä?µÊ­#¬Zü?è@5¼>N?²
¤ÂÄ@?´øÇ.U½r?¤rÒEâ¬@?ĂÅwmõ§?¬J®"JB'?àz3?r†°?´'F¤?Èu¡(ÉÅ?°cŸ!BðÀ?ÒÐȹ†½?³Ï§·'AGN4FGL J0312.7+2012?åå¡ÒD¨À?"›«–òÀ:ý=1¹¶pÀ<xŠ§ŽNã@!²ŒÙÔ?û/ä^¹É»?ϞîؐOn?Ä&܍µ
?øI¢@1Hw@o˜Njò?Ûª%?éÌ"C>C¿àMLïœÛm¿¨c¦¬D¿æ¤ ù¿×¾ ºKUNASNone3FGL J0312.7+2011?ïí˽®!?XLuBÜýQ?.Â62ǖ»?&Þ,€'µé?`÷¹|á?VIã5àZË?ïÜcÒ§&?o€F1 µ?9J8{_Ä?C˜d*>X?p9sAde?lEo=VÎ?á×ËÙ?zBß^êX?Sc5fÞk?X5]Bšì?†£"äÚ?yÅâ?ïr£âƒÿe?n¨é;ïúŒ?\0érQ?BøŸÏ%l³?Ðê:\L{?mlI~a?ïÜÜ?d!›?d¡™j7<ë?@nV)b‰4?4È^IZpz?o*ß8G?c'}Ü¥?ïfHßB?Œc§W9¦?LkO´xÊ«?Xë™,??Šó±€$¯`?‹NsȨ?ïNwe€ý?"Ÿ–@›<?XÁ"Ž…§ê?_2mÚ5?"±·Èƒ¼ã?"]×4þ?î§zع?&?‡"ë
ΰÀ?k°¸üT´–?^=OÔòÈ?£ÍFáU?†ó·ÁNž±AGN4FGL J0313.6-7508¿î踱jyNÀCd0 ±»ÏÀ:Äs'ÈÀ<n
Jk^@W)ªs[—@©L_T#n?Èôc>¾¬¤?…sÐ -5Ý?¸ñ›8U1
?úoÒ@):â¿æLœ[ùŒ¿æçeÕFîÒ¿ë"–Þ(i׿ê+ÿ,›i}¿ïÿå"m/®?ïný
Ý8UUNASNone?ïðœÑÆ?a%†Ûß4?7¸PüN¸k?4rvïò/Ö?Yê±É@I?`
c"É?ïdÑ9TE¹?—§ÑF­Y,?nÏXŠá?w ÓkÅÅ?ۙc¸?"ª~0L?îñÅpž3î?ŒÛ‹¥'Õ?{ÒA췋a?ÍGTÖµ?šÒÁu¯W?ŒC›n¦£?ïµ]gd=A?iUG``ðµ?`ÇÖ	‹ÀÐ?PU[¸ÕD?|ía6›?e
æFí6'?ïámŒå?o€Å\{Ž?Fó'p®é?GaJDƹã?hÕ«¸"üj?mF©Ïs""?î>GÝlá?°Ke3?'¡{ÿ—‡Á?•?¯6q¨¥?§uü}áϋ?«
ÈF~Š7?îdÝ®áM?•%^¡ZŠ?ÔFø~?€ÞB¨â…ó?¥p°wà‹?"?ð‡œSú?îèeôÈá¨?šY¥;M?€1'8Å ?vì¥ü®î?šÚxQ¸hî?‹Ÿ»=J'AGN4FGL J0314.1+2827?ï$*·8¼À8ºH×à&FÀ:•…ú€d>À<³ûD¯\@éeSi´@_yŸÿh?Ë/¥õrˆ^?À¬°Í'Åj?õ?|Ì@Sp?íf'•ù?ÉYF˜?ÒS¿ìr9}û•¿ÙUkÙ3¿áa?èÅQ¿ïýç¡åBUNASNone?ïrïÚªP?ˆá*º¯7?c #Ғ<?a['†­"/?Ž'áN큁?†ßLÀȾ'?ï‡:[gý?†]át´
â?itÒwÍ??s}k^"?‡Ô4—ƒ·'?€PêâGl?ìý`Ý;c?£"¤5t™?Š"[¦p¢?…‹?ð£4?´Â‡'VÒ?¢X-Ç2$?î"d‹šÓU?'¬šP™b¢?€%?|d!?dÙîs
²Q?¢°uùãM›?€¾àv‡ü¥?îÃù! ò?œ¦û³¾?§®o"…‰?QъÊêb?Ÿ–ðEB—d?˜}"àÿ?î¤U«"T?¡Ü3⤈2?€¼O¬† ^?'q\,´f?¡‹'^°¼*?›B9l{?êðÏ
•?°âöÑJce?›Í+´'-?'£¹Æ[D?ÄKö–¨V)?°#ÆØNݟ?ìŠé±? ·Èî@Ç?˜ÙªhºM?…¾`­§´?¹ø<`zá?
ÊìõL£AGN4FGL J0314.1+5033?î"dƒÍaÀ—
€Œ'ZÀ:$²øæ0KÀ;È5"_õ@c«¡@¯X}o—h?Íé>]ˆÇ?ÓÒT`ªdÃ@ÉÅ!Ý @¥9Œ=»w?ÔZÙa?ïꧾ d9¿çZ"zy¿äà'÷–¤ó¿ð?ïÿR[§UNASNone	?çÍô±k?Ɵ›ˆ©~¶?–"€WÔ'_?"†èÈóþ?Í÷Ÿ«£Ô¨?Æb('ïÎ?çü"×%ýQ?Äã	š]ŽÑ?~$ù'¬i?'ÐA÷D?Íþ(Õ!°?Ãɕ•~
?èa…gCÂ?¬Æ€'ÃÑ?°o-5A*?œ}É
Çû?ǂã_5o£?¨€º 6|?í`cJ'@Œ?"Ê$ô"Ÿ?–Þ¦DLá?|Íly4Ó&?®Š¾†ú4Ù?')÷è\ßÐ?ä¾?;"?Ì=wÿ.ã‡?©xžqKšÿ?¨º¢ÀÄ1Ç?ÔÅo³
«\?ʸ®r°e?à¥0|'K|?ͺ›Ì¬o?¢'P¦ôg?«¡nyU7‡?Üc^}ӄ;?ÌÌ¡¬–)*?ár\¬†ä¿?³04Ë»_?¼çIBò¡{?£¤&¯O
?ÕátU"­e?²CŠ¶€D?éÄ+²ä'?«­qC¯Å?¨Òŝ-?"!á&K?Âêß<;²?¨ä±ûþ"6AGN4FGL J0314.4-4805¿ßúm˜ÀK¡cÃ÷bÀ;NüÕ©À<èŠF?@çÖA•¡'@ ê@{S?ˁ.(\j?¶Â\ÜNõÜ?ë²_~ØÕ@–É—
MF¿êm§¾Šà¿Ç­¹v®³¿äömŸë˜?¿ÜÂ=|¸7¿åÿ‰b"ʨ¿ïÿýF\IUNASNone?ïä^ºÊ?W.\mîâÎ?4µTý…?$囹_ò?iT£Ÿy?U¬´5Ÿœ¯?ïÆ=š"?th€¿ÿo?JÃàǦ'?Oóì ],æ?yˆÿºØ%?qédõXuM?—#"?rÉ¥A?ÕÌ?a‹<?ž?V§µ`Q}ç?‰Õ÷qOÉM?q÷h:Qº?ï¢8®¿'õ?bÄw©ZÞ?Y80béBE?<ñ/'	0ß?"JÎ>–°‡?a)«Â‰…?ïËïÝs
>?föt?Aÿ»K†YÆ?3œIUO̅?wÈ¿°¸Ò?e¡¾:«Ò?ïY¿®£Ž\?'¿Ÿ"!?[ ÞÆÄ%?eržw¶°?"ü@­Å ?Û?g…0'?ïB
Œçã?}6@­fúd?h¬‡àB :?e_+Ž¨?"©,+#'¢?yfm_cn¹?ï¹¼{?€.½Õ#˜?kAÈ	_t?Wó¢Õ§™¼?›À£( ¡?"Ÿ¢ª1ëAGN4FGL J0318.8+2848?ã$Ê×^À7×UÿæՍÀ;)-c™ÑÀ<¿¹üæp@)Ç`|B@Á#>?Ù	E#¿¹?ïáµA•Ì…@ë¬c ¹I?ÿ'ž=BU»¿ãLYàF&U¿áãùÚLQ¿¯üòü®´*¿éíô?,­¿ïÿ\ è,û¿Ëƒ–¸h¼­UNASNone	?ëCü{ˆ"?¼FƁá¾?³¯Íi	A?±,IËUG?´>ÌO–™Ÿ?°
Dñ}"†?åG!Q´R­?ËÂÑё?ΌRÐÁ#?Ç¡iòŒúÐ?¸®OÓwÂÌ?±°\@ØP?æÇْ¥V?²¼ÁJ!\'?1"!µ‡?©ÄUìÂ?ÂCh!HòZ?¨¸(V™r?áåO­ðÇ?±tñ܋7ª?ÔmøÏ?®¼ÿ)ŠJÄ?¿!Ş@ƒ?¤DNõ¨?çW¬x)Ä?À¹µñýD?ÀpUÜ2?µ…ÀÎÛ¨"?ÂÝÉ|é¾?¶èÌgw2'?Øæ:柠‰?а a3÷~?ÜÆ`RŒP?ÑÏöÖi6?Ħɋ']F?¼èD'CM¡?áˆJÔåu?¹'¾íE{%?Ï®ÑS)‰?µŒÓ»{-?Ê0Yb:?¯ãBå?ÐÊ?ÎM§¤Zy?±=¡0/ÖY?༸0ø4H?ºŽ+Qg{º?οw—ĵÛ?·"Çÿ†ÔMIXED4FGL J0327.6+2620¿Û O	—GIÀ8¦°úß.ÏÀ;E'ømd‡À<—ªÉlÆ@!B`E:?üž×¬#ßÙ?áò_£Ô†?»ãâ½úÌå?ãe	ÚtU<@éBb{[?î'ϝ+õ¿èWrþ$]­¿ìJ-J»æ?Óºí¡Ç¿Õ yó$÷¿áâ"I΀+UNASNone?ïœÜê·î?²_@àÎj?9+Ûì-)†?0ûÉ,õ_?‡ÿfŒ'Ù?q¯›ǽ?ï¤ÃòfB?…'•s'•?Y='paÝÛ?c7¿"Ùãz?ƒ§^zsˆ?ƒøE±òú?î_Þ=sº?›!2ˆF¼?bª=ºxqä?l_¦û‰‡?¨×xHýO?šÚº?7?ïM'ëˆ,g?{4²ú¾v?DµÏçO‰?8†Ù€zxy?•§ôàÚ?{vØ̤Ò?ï3™??•ÅV†«r?J¶£¦¸Rf?EF'À}²e?˜ÉȚêк?•V"'?ï,êI4|^? t\¸¦³?a@S•Èæy?uŒ=Póz?˜:¬m>™Y?Ÿæ c€`–?í¼«w<¢s?¡¨ø*uSÒ?c@Ñwȋº?k_"$0n¯?±€»…?¡ ÄßýÞ?íÎ2i"?žu³è"´M?T©A>'q?Z]Ñ (—?±;È`´ÿ.?žV´"Ï^AGN4FGL J0328.4-4736?ï—3÷÷ÚÀJ¢s-õÑÀ:ƒ®E"IÀ<µ÷ڗ«@b±½|ͱ@¨¿§J\?¸ÚÇ6_ãj?"O®ÐËS?Êß«6Os@´Íí^<Ì?Ñ£ø'Äj¿âõmÕÆp'¿ça"oŽ-¿â¿§µ¼¿àá:þϾ¿ïÿþR€ÖTUNASNone?ïö<f|z"?I…eÂÚ?+‰ýèVJ? êžnëp&?Pó¿ýFí?G
(ÛÚ<µ?ïëy<_Š?eáHyÕOÆ?-F8°­Z?;OðI°«<?c#9/ð?c¢ïô¼l?ï°©5÷f\?p&Î6¶uÊ?Sûz£ùޘ?SŸYäQÖ?VC7ö?mÈÏfØð¨?ïñô{´Î¡?9}ìýÆݹ?4ЬïÖd?ž"û¸÷?VâÝ!Z ?7¢ÌY?ïâl»XõÔ?d»â!{Xo?Bs"X©?6žE?&Ñv?höc«jaQ?c+Ýé©¡)?ﻧ¬½ôÔ?'<‰:A??Ç1	?Pú"äSm»?€ܘW\V?ùw*?ï\;ðú‡#?"×$ø½ü?_¬§ñJ?V9MøFÓ?'}¿ðܦ©?ƒºv†ã•+?ïÛy¨u?WªeY4œ?Lىé"´G?:i$'–æ*?m¯#ëSâá?U»LAGN4FGL J0328.5+6114¿é0enLls@`'ßBñÀ9¼.±Ä2ÊÀ;wÕ<ÝÖà@¼®'úï@í`Á
ø?ÇV–$D-?ËÕü3Ã@B`Û*±@ÂÅ(=¶Å¿á¥‡
¥Úð¿·<Ê5ñE¿éÈ>O¿çÁ‰¢«'¿íÒEb	àT¿ï©œQ3¤UNASNone3FGL J0332.4+6110?ä¦ûIŒæÙ?¾8S%
x?¡=,˜Þ_?›ŸeŠ ê?Ԋg'Ÿã?¼™Q­@q?ãà~ôí$?ÇIþÚC¶?®F‡~?¨Y<ýÏ]¨?Ô{ 
Ą̀?Á+ÁùÆ?暈}:œ?°GÈË[>²?ªÅˆ™mÚ?–Ë÷³×è?Îä{æ¼sJ?­Võ™ñG?çþ	æç2Ý?öñìõiØ?«Q¶›¦òÅ?'ƒä<´H?É3j½°qš?šÕtzÌ?×p¸­c¯?ÀaÂٕg?µÊõøŽHb?®¢Lôäé°?á¼häÎ~Ü?ÀɏëðÔi?ÖͱËOR?Æ0Ï@D"®?½@¶éᅗ?º€žzBÖ?àñaT·E?Æ[DƒVzû?ÚWa {{?´dípíd-?º²«@W€?¢ò®mB!?Þüµ/n¥?µ4"².?ß/¶¶?©ør0Ñ?½A4ÏPÆÓ?™˜ÉšP>U?ـ­¼ˆ©T?©Ç^ERMIXED4FGL J0328.6-1129¿ï‹]v}µ¸ÀHü«`kz¢À:Òe1³sÀ<"½	á*R@ONœÆ@)ÑÀQ"G?÷:ÿ°Nè?'–¶q2?ϱ^œÃo¬@e-a4l?Ï´UªV€¿è—ñXP¿æ?ªºÔ¿Þ墜!´0¿éÙßÚƋ?ÑZ½:ÞxUNASNone?﨔B©À?z›qYP½?U´Üyë¹Ú?Szg§:‹Q?ƒ$_¨|À?wwÇ?拓gpI?€ÀxHþ¯?X"eþ)?^7LŽù(ˆ?'Îä+ô‡Ÿ?|¡p¸WÕi?ïdÖÈ_?'2dÍ:?cêŸô@?`z©:?'
Çù/T¢?}‹D‹µ?ï]I{bæ™?pÇ°nš?ZÅDZÊg??GÜÉÎo¤?'ª˜;íäA?oWÁ¶¯Ü'?l^^?\ïöñ¯?iX;²àöÑ?[´Û"µç?™ãEdW%R?Ï.vÁð~?ï1D¤°à?"Üt3V?a£Ù3Æ£?k ÜϽW»?—¢ð>ó¯?"'ÌT€* ?îÓ¥h§*É?/ë"'?p"¶¿Á_Õ?l¾`'"ò/? ÁRšQ†x?‹Û;íšaf?íâÓ«p?BD·Ùº?t\Ùǟwè?aêŠ;m?¯G*õ–ˆ?àº[AGN4FGL J0330.1+5038¿ç'"ôéBòÀÉHýŸÓÀ:!2m:•þÀ<º«bú@Ó4E@äÀ§$?ÄBصä(?Øü;Ú÷‡á@n¡žJÙB@Ú²šF'¶¿Ù²^ç0¦¿Ö¥›E]à¿ãí¿@r5ý¿ã•#þŒãS¿í«&[´\¿ïµëÿíáoUNASNone?À&ϓŒËf?­âw31=Œ?ÛW¥F(¶á?ÅÖiRBܸ?ܔòðãl?Ãzâ>¸3?Ö3ñî‰#ï?Ã>í¦ŒW?»êÍdˆ{ö?°7àuW?áh­\*^Š?ÂéÍQY?×Þ{²@Ç?±ãÿñ̽\?Ô'&MOFÃ?°úËØn<?Óú^¢xw?°§xs}?ã½é¥J§Ä? Üb@¤Ñ?Õ1³‰ã?—uW½M >?ÍøÄ6ü?š5¶fK<?«<Ätê?›Î§~Ë?ÛÇ`"Ø ?Æûf™£:é?àÂÛ/CÃ?Å偼$«R?Á\Hf‡Y·?¹O2êuñ?Áèq<?º|ñÿG"Š?ç.ї6èÊ?Áç,–îï?ÉÇiÎOŽ?«³q€ý"¶?Úÿt4ý…?·Üà·ë?ØC¤¼Ú´?µ¦åÞ³Øt?Óói7ëÃw?¤'	V±`·?ÑpJó:Â?¨Tdy@"?ڜ†|!	?¦@I°ò)MIXED4FGL J0330.7+5845¿áâåy'Dy@-Í9ÚÀ9wb§•À;4ž"ºåD@~B¨œ@a¤_Æ9?ȈªÉlÅü?Ýøk¡Ž°‡@h£?4É@3:·áÙ#¿à6€d¿§ŸÑþ =¿åÔÀdïn¿ï6ci[ä,¿í"äEV¿ïÿç<t%UNASNone?Ìy¤¯è?¾:®–Y?Æ·ŸÝ6ä?»(b†!?ã3¯Z†M?Ã2®lÔ?ÊÚô:?Ɵ38³ó?Ðñ	Ô%lÝ?ÁÑ^{z8š?àÐ÷°;?ÇRÀr²‹>?ÖªTj™¥?±ŽŸìI2Ý?ÅXCm½ó–?©•'d?Þ©‰Þˆ?²9<¤BŒd?Ì,'È~	?žÞaÍ4?Ðû"žÅ?¡³N£0"?àwJn…'?¤Ï"$–?º}
¬+0?²ÜXJJÐ)?Ãg¹Äÿ›?¸–¥òŽ?çíDÐÙ:³?Àƒ°ÏQ?´Ô›Y S?»BZÿ'+r?Ô!5¡x?DŽ,}•	Æ?ãT­#FŠ?ÈÉûZÉÇ?Ê[ý×Ër?®iévÖé?ÇÍ%löùF?°,TK›T?ãuñeÕ¿1?´Y%"ö-?±Çè¾±0X?3ãRw?Õ-ÊAñÖ¶?¯Æ˜>"ö?ã0Ǒ#©?¯å[¨·­OTHER4FGL J0333.0-3044¿èPQÞçMúÀKRxá"-oÀ;MœÏڞÀ<Ø´*>—ë@FdV@Ô\?ÿ«[˜­
?ÇSÀÜԁÍ?ªhm&ÉîK?äÏ Ä0@©CU,¿í¦M;òõV?ïýR¦–_¿á:ª‹Ydö¿àH?xæò¿ç/jñæaÉ¿Öф!bPWUNASNone?ïï"÷jžô?™b3~?40szYŸ­?u¸z-	L×?\­ô6tŽy?"ôGP{·i?ïæþúúæ?i[ΆÛå?1…­T~\??ۖק"?fÐOE²ñ•?fʉ\ÿÅ&?贈…sj?v— 6i
(?PŽ)>‹Ø›?8îæSŽÎâ?ƒ
ÙyðW?vS{X¸M?ïÜÊDËû°?Okë%hõ?<•OÉÒàU?"PÂëuTÙ?o£kNø?NsUíZQ~?ïê¥Ç
§4?Z¦ïuÃ?:¦®ë?	?3Å0‰Z?bcáq²?WÔêžàþx?ï®Äç®®?ƒe%‡ò§Ñ?EH+fqN?[–І~«u?'ýƒ#Ë?üãš^……?ïj:#}?'<ؚ(¿K?W}¹ 4?P·^Ý[?'@╮I÷?Êà¢c`?栗"
:?jfF"3D?LýYéP?</½(¡™?"I…`KÍ?i½àÄÓ
—AGN4FGL J0333.4-2705¿éªÓ>g*ÀK¶"‹ë[À;=`ðà:À<Øꭈcç@K¼À('?ÿÆü9¡â?Ê}v"q?®†‡™'?äh][Œ@ôôÕ)"¿ïŽÄ¾áQ¿?íôÝ!®¦q¿ç <4cµ¿Ä{ÿÀ?пåÝÞ!ÞÌÿ¿âÆV@~uQUNASNone?ïëçʳ?PŸÏz?,gôº»b?豨éÉ?bQÃôŽk>?Ož{YÅ)?ïÞDäû?nƏßò"?:¤³lÊÿƒ?E''!å?nf…n_S?kA¬D?ï†Ì…Ý­£?vÉeL%–"?ZŠûU¨&p?F"JŒ+?Šûoöf?vd"¢Œxô?ïÄÇ},¦|?ZÙŠ"^?Q.H3?6E‡kÀ'®?yP¯gX¡#?X¶¿þˆà¨?ïØêRwNÊ?cç÷±¡?<(£=¤¡é?0>ápî?qÈL'‹[?b£'Nö*?ï'%ûïÉ?ŠÁ…µ¥Ø†?O5>P$'×?bOÌgv@?‰Ã-\qªn?‰(Už<øv?ï;Âûà+?€bªUâ?bØ'u/?XIƒ.Û¤?–/-‡P*‹?~ælCÃC?ïoHNg/ÿ?uWBrÈtÐ?b¯âzðÌZ?R´&šÁàQ?óԆQ)?tˆ©ÖTjAGN4FGL J0336.0+7502?Úö NB@/DêÀ9ŸÏ!:ã+À<Y›0r@\kæ­ô?ütàaÕ.?¹	àÔk§™?ُ/Þ?@ 	ó蚈­@LŽ\¤œ?á%âØo˜¿ß¬übf§¿ÒQþ$ˆ x¿áQ"²ªØ¿í*ÎuCxü¿ïý/k'–GUNASNone3FGL J0336.1+7500?¦@¢Yø"?¦Ÿ¶žu?î=é
 S?ªAGZøî?‡ƒ2'³?"½u‰ˆr?´bÇêG®?² AÙW?ê#'4ÕÓ9?»L7ÀO´?ºƒþo垳?²Ú@߶b?³CâömW?£Oö¸X¡'?ë2ÔjÈBF?«q¤¨®nð?³%y±þ²{?¡ÔD'
–ø?ז{½Àg?ª4Ácô,s?ßoËGš&?©ûðų$›?œ(ïQJå?—è?ìw?œÒ½U<?"g¦ö"¸?î³/S™sô?›·4ûƒpB?‰Ž°rÔ&ì?"s×Ûö?¢TƼšH?£Ü×ô^'?ë×2RÚÕ?¹§Ì¢°n?¸?Z\8?µ/¹•³<?ÖM¾Ÿ™€?•­ óLî?íC«®ø"?£ueW Ð?¯pžbQ?œ_§L¸ÿá?ÆÒ<$•Øç?¤ŽÂR¯×?ã'kn?®¡ëA"æP?Ë%{'¾%b?£<0Ót–1PSR4FGL J0337.5+2423c?Ô;¼9ҎÀ8½ëcÉÀ:¨—,ÊÀ<E»,'X'@#:´†ÚÐ@"WæpâÁ?Ç}–™4?Áo,ž¯N?öŽÞ9ܚ @(Àr×
?ïï"b*—ƒ¿Ù£`rpá¿åSj
_Õ¿æzˆ\Zsê¿áåO_¹£û¿èӎg.UNASNone!?ï†YÁ'´?z°g=à6?S_1s×qx?JA`­÷Âí?‹ý©šŠÞª?xn9¥-m—?ï˜ä1º¯‹?ï°Õ¤Î?`Ӗًx?aÀѵuˆd?…'
Ês??z²%۟Œ?ïS¸{v?{ÆM›ƒ?gA
óxQ?\©H™7þ?'¶/wE?y¿o˜Œ?ïX'"@?n¸PSSˆï?o¿Mè&)?M"¾,B»ñ?™ñUÁs?w?m|Q=?²?îՃOÞÃ"?
ôö'?jƐì)'?bx6oÃ$_? ûj«*ÌÃ?ŽÜÀf¶8?îè
¨¬B?š.†bµ?rNXCáÕ?~	—Qïw¤?žk(ÕÒ©?–5$ŒÜ…?î|£FÁ…q?'E¥ðwÉQ?z G°²'?q¢í?/b?¤ôg‰e¿®?ø&5×yå?í*>nª?‹t4µ]R=?…o­#`Ä?nrƒÄßÝ:?´)¹'w•?Š°…7oªsAGN4FGL J0340.4+5302¿äÐD<'׿ý&^ê–À7½?R%gÀ:ÂÊC…Î@ŽÛö¶U<@Àìœuìì?°¸q`•l
?äéÝ~Ë·ú@*Q)®O3@ÆÂûè™1¿½2t†¿ãˆnßßh¿í³k¢Š¿ï"Ú'—õU¿ïþT~ÝU±¿îmõa™šUNASNone3FGL J0340.4+5302?£¤è»Âm¶?¹àFøÉ;?í0/Å4?¿ØÂcè1Ø?©ZäGÕ¼?²ÄMíÂÜ?õaÜâñ1?©&ƒOâÅ?ê–Ð(ÌÒ×?¸ºNVô?ÃÅi>'?µÃLˆQ©?ÉVUAzô"?°Dä	Ð{?âèóÉæ¾?µk¹È¢?Ìjñƒ1ñ?°Ì#'Ü«Ì?Q!ãV[i??öatT?î,ŒjS}M?'D
Á¡¯ï?¬®hK­xU?'Ĉ/º?¶"¯ {?Åß5'ÿ"Á?ë_F.?Èè.° $?±œ>¼¥Ï?·ò4@à?ƒé»á¾.£?¢ûBÅ(g?ë\¬Áó¨?¾gE¸µ­e?ÁN±9¯ŠX?»ì¸%Œ×?ÆÙ)äR?²2-ñø"?ã|"0;?¸¿›zF!Š?Ë6›Š,
Â?°­Ù Ôå?
o_X"?º9wI?îá'rƒ«?ÄüJžÐ?¡Úâ!8X
?½÷@¢aPSR4FGL J0341.9+3153c¿ïÿúýóÇtÀ2]`—ÌÀ:4NƒÒÀ;mœzª@/¿@÷C[Ÿc?ԞLœ:Þ£?ÜÏí]æåþ@âyWòÔ@\ò´½âN?å¹ÛÃà•?ÜÙ&wc
ì¿Ù5ä=Àµ¿åÄîs¿ïýà€ˆÑu?ï©ïÝÈóyUNASNone3FGL J0342.3+3148c ?ØO¿Ë²p€?ÅeÜ'~~?£Ÿ]…šË?ž¦ñé3W?âž*A¿_s?ÆKOÿÇ é?íͧ3ځ?´"é^ßѐ?1ÞdóÌJ?¥({º?¤Œ˜èÕÓ?­½xßÏXÏ?ÛÜy¶'ç?²Ì´2:ÿt?¼†pƒ1	?£¡n ÛG?Ýd­\L»?²í<??ވ‹Ô"ñ5?´4ï-Y[d?¥äPBªÍÞ?‰Ñºs•?Þºê#l8/?´Ù*J£´?нÎQ?ÁBÕÈI?²ÜÔÏøÍ?°aòà[¼?å¡~…}>?ĶŒˆRä?éHÎ6?"O?Ř®Ù^‰?»:Ö.#c?À­ü_)ö?º~¸tB%?ºc'JOb?ÖÍ'ò0_?²BwùÕ§?½æö?s¸?¥^þE¾»?àܔï"º?³Ÿ®ëí"?̲kF8ã:?²¼Ù­KvM?§ LÖ¼G–?–ê
ž$?ça`aXyX?µOáÀe;MIXED4FGL J0342.4+3125c¿í…)Ü-¤À2©Åæÿ}úÀ:Õ@8ÕÀ;x=õ.æ@N‹Ô4@J·'$1?ç&
{ÅÕ?Á6fC€Þ7?û6jŠ¸UG?î`
­¿&­¿Û›ã`bt¿ãôw JŽ¿éÙȓ'(d¿è«Ë*5]°¿ÐÝg#Д­¿ïóy^æ•KUNASNone ?ç«¥k¤v?ÈÖýN,Ì?¡2lEÅÔW?ÁÜ @¬?ÍÏA5T?ÄîY˜?îÂY<[?ªS¨´ÃV?‰ËEQÔ?–gÿÙï"?šÏNÂ
 ?¥ø™œX?咷›ÉZä?°mþÓ˒½?¢'1'åž"?–£'Z©ñ`?҈J–†?¯vksé"?áaÿ0øƒ?±'ãGè•ä?ˆÒ²…qñ?€[Ù-Lü?Üul
6²?±\A6'?å\v~jÛ?Æ¡8–ÁÅT?£ƒ,¿­}È?¹ÓÛ(±`?ÒÖ­kˆ0?Ėò¯å`?ëš1šò™?Ã/Š² #?­6¶WaÞ?¹ñŸo:ƒ?´"µo¯?·ü:Ic1?âxYš™?²(ށ¼>p?®Xç¡4'?Ÿm`¼¬?×D¬Y‡'I?±±I"³wt?Ñ{.ìÉä²?·¡Â8…hÆ?…@öŠ¬?¿œN
ä?æíh1Ü_×?·¨ëg~MIXED4FGL J0343.3-6303?æ½ì$´rìÀFF	=–c"À:Ÿ–€	¥›À<¬F<$s}@Á²2l¹½@b°~¸lÃ?¿Ù•2+Ì7?©wDã'i­?ë™þ^?Px@¨S¢ivç?îg‡=¡v2¿çÍMZü¥Ø¿ßçÚ$#JÞ¿ä~q f¿Úiœ;_|'¿ãTÝ<†™UNASNone?ïÞB,£ ?]1ï­Ì¨L?DÂsjû?23³Œ@?l6{fy™?[Š§[A?ï¶!Fœ?x›ë ¥ç?QL3â"
?Tz\oÉã?€T…ºŽ'?uÀûZñ=?ïÛ¢¨‹û?u"2I"Kº?`¶œñ°?QP¬Z±e_?Œé¢,ò?t"'c~ÜR?ïŠ?A'ùE?fõ›(D?a²2ÓÎ?C'°^‰ÈÃ?‰¢éýÉÀ?e[Q9úfÕ?ï¦'xc??‰áøNw?]]ZŒ³(?Rçî€ÿ²?'Ê"¬ƒ¢Ö?}Š¸–ç
?ï=ì÷ºŒ?éåÏa®?^s,£?dê
ôplß?–f°µ«M??ŽÕiuÜÈe?ï!è¡ÙH?'ð]È2‹?j	°èö?`èýr¢þ?™ŒÕ-Fõ?O^}‡ìÓ?c*6?ƒÓ3êKau?v£3A
 ?c"…Bùê‡?¢j᫸¦?ƒœgµ¡±AGN4FGL J0346.2+3235c¿îÌ`"à^À1?&9O¬æÀ9ç"gnÀ;ˆ®¬Ÿ0@À}ÆC@FÃ1B˜?Ë=+¯†?Êr)H!@Y)Ù‰t@«;[ º ?î/ŠÂ;N`¿Û!ª	SeÙ¿êÜÕÃìS{¿æàáVÈ¿ê3Òê¿ïq"L["fUNASNone0?í›";èq?¥ˆi,J~?{µrGÂ?t‡¡î&Œ¥?±nÒÏ"ðù?¤_@IŸšà?îØÄ!#´?¡c,x˜'ê?Š"æÞD9-?ÚŒ£Èä¹?—ÅÚ5?™åƑöíE?ë­íŽŽN?¦gw…ãþC?›xâ8­é?rßÐÈu?À,ùjÌ?¤c¶ûؒ¤?è³Ü&»?™‡øºm
?¢•¾õqý6?|UL\×ËÉ?ȋ¬ b?—"ÈÇǎÑ?è'Ë­h?½@ÇÑÁ?›És•½°¿?""‰³t@'?ËèZ^'©Þ?»q£*?ì?𵬗?ºòÿ&_õ?ªŒ†?±¸fî÷o
?°º3…"/?¯§Íc'?å.ÉCÖC™?±ùjÍöÞ?­ó¾òå?œ™UE¤t?Ñãõµp²?°ŸY/l?ÞÀœdœ"'?¦æÌ}ã8?µÂxËv?•ó×ÖC?ÛÎÞ=<Ü?¦¦\ц(AGN4FGL J0347.0-6400¿¤:£E
'ÀEÚà"'À;¼qáÄ«–À=_@©={Œ@?²õ`>Ú@D@¡±?ÔaÝÖ	Œq?ïpaêh@¥€éŸk@óĺÇ`¿ìolÕp«¿Üޝ"µ²¿¸®ƒ5ªø¿äVˀœ¿ì°<]ÔF"¿ïÿÕ"[ʁUNASNone?ç§N•,¢?ÁdóiÅ?ÃImX]i?º×ú"¯Á?¼2´{Oà?°·7¶»î?沇Aßs?Èi¾_¡¦-?Ç|¤žããó?æäÑõ?»r}Ð)<~?³IIåí?å…H Lž?´÷ÜQ£Ä?Éñ{Ϋ&?±ŸˆÒê ¯?¿òÇa—¹^?¥7
Ätõ²?èDêsYr?­ûó¾Äš?Èòc¬šÇ?¨‰Òú÷g?«R"§=ÔÉ?›fàc÷Y?ã¬jG­¤Ð?ÆIs'ì?Ìþ=?·?'Õs,u?ÄP¤Rˆ?·6d7"s?ݍT¿Å?ÎðN²º¢?Õ~¿"'-K?͚½0!°Õ?Éç×µ^>?À&?Lú-?àÇH$Ë«(?ºº×Šs"€?Óã@?í÷?ºzÜ6™'ƒ?Å^î«wp?«7J\)'•?Ùâ[†ÛÉ6?º0^±Uí?Ý°Aíœa[?ºÐ°Jú¾ç?ÀÚŪÝ?±Â†%»ªMIXED4FGL J0347.5+0722¿Ì¯ãGˆ>ÀA"åÞÊmÀ;oH-–;@À<šŒq'êS@!'µ~R?üÃ?ÕØå	?×ÈÛîBé?Ôò–'•¿@µŒ>gCÜ@½l‡'±¿ïþØþ^jD?ïÿñ‡—8–?ÙËëü<üá¿ËЎxSMÛ¿ÌØâ
ü˜¿ïû|b§,UNASNone?ïÃkÙå±?t\F'«?Q"eé:'?J—UjÇ?zâ-\.ª?r˨Us!?ï¡<H/Ĕ?…Ú[±Ÿ?YøºËrK£?dþwöûÚ4?"qÖ§W‰?'€Æ•ÏUU?îš"0£¿?˜a¢¡¡?'Ë)=¡Û6?‡i-_v?¡«¯-uF?"9ÛÀpù?ö£
?"0(ä;-œ?cõª‡ï Q?Q"gu
ç?¤…µìHƒ¡?ƒ³}×*x–?ï"?p5û˜?€tq¶…Ž?bv¦ð°.ï?ZÔ9$§:Õ?†RzB³¦-?~lBhT)?îö²%£õà? %ýl\1 ?iaÆßñïP?vJ¡gÇ?ý'sΉ?Ö׏3ê1?î‰{`À×?œ	Ȩ;M'?€(ä–ë-ÿ?ƒ$tGàG^?«m/!cy?™œ~øÿ?ì"WòÉûP? ¨^¸ÈÑ?pyª¶®o˜?i>ÏD0'"?º]¥¼VvÉ? {×»^AGN4FGL J0349.6+4026?Õ¢s	.tTÀ%GMƒAÀ:m@OÁßÀ<òö,A§@fdzÔ@ý¡Ä
†l?Ñ\^¥§ÄÖ?Öf.Þé}@;¹Ïš§@,ý ý{–?ã.žxük ?ïç¶}U[¿åçð¶6¿àH"íˆ.7¿ïÿøÞ£Žæ?ëóæ·YžUNASNone?ê'3ôÏb?µØðÏ8÷h?—²®\'š?‡æÈ?ÂÄÚ`ÅMä?³øÇ(À_ù?ë:ïÌùdÓ?Âp™)v
?šNŐ‰? ˆÅ>–œB?¿"Ð10N§?À±÷çá.?êKjÂÊ#?«AV/¹5~?§ýW¿e£K?–{<ÿh?)?ÀÒÿÇ(ã?¦ÿµòߓË?ìï˜˜…?"¸ÒQÂ{?¡veÛ"¼H?ƒý™þ@V?²ÅPKòdz?@âTe¶R?åÈ
—º"²?Á¶{Ið?¨ã$ä!8?¡žò=¸?ÑoHkîTv?À'Ý^P©w?çCÑýýá?ÊÝPÙób?­üAõ?²©ß[?Ëq"F7`®?ÉàDp>Ï?å#WÜ=‹¯?²òV™¿¯?´EÒ¢BÃF? <Ò ú •?Ч۞PÑ?°Wdx4 ?çè†g¸ª?ª<¯ÈB?±Q"	ß=B?œ¯e·(›Œ?ǵ–òR÷?¦¾RœKGAGN4FGL J0357.7-6808?è¯î(MbEÀDO
å6PÀ;ÏrÎ\À<öòB9`@!Êy»WÚ]?ú6?Ýe¡E?ÖRÆ«ú?À£ÇšÞ¾?붖à+Ï<@J÷ñé'Ô?àq<þ¹?ïÚÚA)•û¿êòø°€eì?Ì®‰•Àq¿æ۝ }Ç?»ñÿPUNASNone?ï㿈t5å?]ô·çÖE?-Öÿd|fæ?%Ñq¦²?jcÓ[KÉ?\éÖPŒ½ò?ïÔÞ. |?t&¢Ñ…ª?@\Š#ʇB?Pÿè/7?s…W›Yü?qÙNZÐ?ïMÚH¶R7?…%‹
ý¸g?`yZàÒbk?dÂ\›b7?"5‹‡pÚ?"HǧÆni?ï¾}iÀÁ"?g5Ã1F¸?Mv½žîX?=¾$sŽŸ?}r­vb3?f6EñUµ?ïÈÊ	àÚ?o±ôÖ¡Ð?B[•Fص'?>Î;Þl€
?yOˆI×6Î?nTTj	cú?ï‡h7)•ƒ?ŠP+\·?P9åҗ>?dw:ÕW ?Œµ~¥Ã?ˆ%=uX&?îûwÄv€Õ?ŒŸúOʕ?d¬çɺ3?m–14ÌTž?ûj|È?Š˜pF0ˆU?ïFÊÌki?"X%¤bC?`!¸[®€÷?\ÙòøJ
?•"oy\"Æ?ƒÕyÖp
©AGN4FGL J0358.1+2850¿Äùy~8ìÀ2[YÿOÖØÀ:÷
"ù$À<\ZéZ¢
@°Áü9L@¿­½=Ñ?Õ¤Ùÿj+?ê7H €(.@.Z¡6F
?üÅÈkêó?íÝ	@¢C¿â›EÁ*WB¿â!'o°'¿ïÿýF\I?ïþÞݛ|¿ïÿý{ÁA~UNASNone?ë³æ¥RØ?¾Ùòû	Ì?§"rl'Ë/?¬±U4Œ?¶—Ö^)?¸¸™
PÜ?î¬	!"Ì?¬1£­mÌ?ޏռ?'·òùpë?šrýQ
´€?£°MU©_?æfÝm•?²­"³­BÎ?Â%ó[Ï+?«)S¥2mÕ?Ä>–í܀¹?«K¦Ü-Õ?íu£Ô—,¾?¡¸Ïxzop?~·Nz%NÞ?€7½éÕ{-?²glt€,!? MŠÇ'?è1d?ÄØ¥¿#?º rÉ­é?».Ÿ`êÞ?Âs¼–¯ë|?¼ï 
*yÀ?ë¶êÀÜ1?Æ8#g¹!Ê?´iŠúÛ®?ÀèîX/8t?³ ½­Ó•ò?¶€P -<?â'5Ü7?¶à~¦ì@ð?ÊáS'-v?´!í-Zû%?́؆ö ?°æùóÇC"?嗵'¥b?ÀۛÇtÚ?£l`í§?¨…³8Ë$`?Òco×1?¾Æ²ù´XÚAGN4FGL J0358.7-7403?è澿)1cÀB£"ý*bªÀ;20:ZnáÀ<ˆ0bžZÉ@e[ç1@ÎàV?̒3ž½ð¼?¦òC~ÚÑr?Øm˵u˜3@fâ(~¤K?št.P}¿•²ù#hæ¿ç,—moo$¿â7¡Â]B¿æb§•¿ïí=±¼PUNASNone?‹žÑ‰?«´£"hçs?Lêå‹BB<?mA´yȄ›?ŠÂîÄǯQ?©þ»iD‰"?ïÇ®)¸O?rûÎ.' ?EÙ¥Õ`£?Nl'lZ6y?yct>[I?p§
0Ñ?^?ïs³"ù÷?xÜMä[?cüП7ß?dӂn½Ìw?Ž<Ÿj?v|Xë"?ﯹ`ß=é?[ÊsT)-¼?RX7ÎN9?3»ïHÑU?Æ Ù?Z¿$ú}‰?ï'(h?'™—2ó.?GbQMüÁ?A¾Ø!ŒÐ?Ž¥YH"È?'g)·™6?ïUg«_ê¡?ÐhUxÌ?X³LEÅ[e?hÓDJ.ºº?"ÇÕʪç'?Œð&ÑÍ}ý?ï
} %
7?…ò–U¯nt?o9¿][Lm?j'V間?šiG•?ƒtÖ|ð?ï$	(aŒÒ?x㇂J‡‹?ewyDÀø?Q¥H ?™?˜ÏëʚÁ­?xÉË¢j£AGN4FGL J0359.3+3626¿ïá\ü°?À)%òE,YûÀ:…¹ª±À<pÚ]¯@$)*Ü@ú'QT†?ÐtµÍ¬Ç?æÛÊ@«kÔ@êyþɟ?ö¼ß2ªø?ïmíCdٞ¿¹ÄÞýã|¿ç¼æ'æ¿îÛú'½˜¿ïû^°d?îtp–kUNASNone?Þª/^…5?Íæ;2±?´=-ù[¢È?µmbœìÛ?ÜF…j¸…˜?Í®ñ‰^|Ò?äð'¼;Á2?Ñe¾Ù¢¦¼?Ê©b°aæ?Ê°ù÷A.?Á"W
`™P?ª•êã?à×áªnAì?³·î‹˜_?Ç­zâþ?«¥yq1Ñ?Òy´î
©?³Vsº,?Ùý¬Ü %?®z -w%‰?ÑeÅRkC?®–feóK?ԜÒ–š?®H&9™Œ€?ÛdÑá^ª/?ÍÁ¶K߅?´¼|ý¿?±ÅÕ·vx?ߙÉïf™?Î>ÉO¥ëÉ?ـØL ¯?ҟáµoÁ?ÙKñAî"O?ÒRZôJó¢?ÊgßÉdôˆ?ȕaé Œà?Ù_C·ºÁÝ?´yP«—‡–?Ï_³èO_?³TEl	ß?Öñ6nQs?¶ûXC?Âý`^ˤ?¥Œ9R¿½?Öڜ'Tž?º£&uµŽÃ?ߦ"¿?E?º
²Ð;0MIXED4FGL J0403.3+1249¿ì	7ÝDœÆÀ<¬€"ÞÀ:èù@ÉìÀ<'ä™r,@VŒè±.â@?)á{?ÀӚÇA«¿¶ QY9S?ö̯UÀô?ú®ä­³,?ì0©€—j¿ê;÷'X	¿ÞH¿nÀR¿éÐ"¢lQ¿ÑvÒîL#¿Úé<+)UNASNone?îdŸÎÀ?¯æ\7Z׉?_ObOh»†?b€‰¿&È?¨»ŒÿŠœ?¯9KÎ{×?ï1܎Y?˜¾Ë۟É@?w
Ôüèd«?¢Á^Ð2?"¸øëŸÝ?"o¬%Ü_F?î>—•]u?›Âœ?zpŽ-¸É'?{©Ìm²…+?«î½Ål?™þ÷¹¬ÖÛ?ë€v½L?œ¹im¬Ö¸?rÜ-(·?b
Kß#Öè?ÁgC¤"<I?œh{c^?떄ç¹jÎ?½Î1¯X%d?|½Ôô"ûý?yŠ:­?À¿ýº,¨?½
@šÏό?틶‹±"O?·Y§GIn?ŠnâЉ	?˜ô"ô1oÙ?°`ÝÆTe?´Ûˆ蕣?ëÞ tT:À?§éªÞMnA?ˆqôb]°D?"ÔNøë̈?½ü½ÑîZø?§$R÷SÑ?âÈÒ]wÄ?³:]¥Gò?ŠQŒÐã{É?ƒ˜SÄ@ó?ٛÏ^¢wº?³.¼¹"AGN4FGL J0405.4-6929?íþÍVp¶2ÀC©= ò¾ÏÀ:'3æÊÀ<q´üÌnÙ@*£ÉO•@mt­P0?»‹/ÉqM ¿˜ßÌȉàÙ?ݺÛGŽŠ@	‹QC>™?ëwA 3fµ¿ædaX"¿éË¢«;-¿Û£J<º™¿í°¥)œ±¿ïÿÿ&¦³UNASNone?ïöt_ç?diccÚz?725î:?KªÂ1¨?La${+?[È÷¥Í'?ïÝÑg™ÊÊ?pñHüvõ?;>ÝB;?GX€«†à?nːÝio^?l[¼—s?ï¿î"À
n?sî['á?Z^ë7ø?dšZÅÚ{r?ypú¹yÕ?nâèóÁÿ¤?ïڂ>½š?P"0ýoˆ?Rp	'Èþ*?7\dGª3j?lEø@ßL?Kõ‰T)Q›?ïïóàâÙT?Y–òF˜8›?El¸àÏ?@׿YM<?UŒ=ñLœ?T¡I&º?àÀŽ?ˆÐÿµ¢ü©?M1/™:?`bû±ìh ?ˆþ&†ÞsA?†µ\5
'‹?ïœí7À$?xÄgmã`u?`'V-Ÿz£?g8\.~iz?"¤xˆ\B?uˆ—¼;Y?ï"Ï9°ó?n4dåH Ù?nñ±'¨?Zމ)¶:?ƒDu+Ï\a?h|©ˆÌÛ!AGN4FGL J0405.9+3041c¿À‰j.ilMÀ/±_$RÅ À:Å><À<
Bð?˜œ@Þg~ê@%
ÌÜ­?Å["J§îò?‡¾%·l	á?Ãî;ÝPÔ@¬G±"?îß"o–Ñ?ï´÷ù¡A.¿ëqM_¯=¿å8׊•ñ¿áýK 'ß¿ØœbÁì!UNASNone ?îæFEŠ?¨}pµ$?pÎé‰P^-?kÓpËÃí?­dÄjq› ?§ª‡Õ+S?ï"M²»?ŠÝUƒ«v?bôdI`[1?oIŒmæ}B?†;"¯àT?†Õ'±ÎL?íµhYÒý?Ÿo
¥?sÅF‰í?zñæ¥ÑŒU?°(ô2}?™P!G—?îMh®j6*?ƒên%©-?|(Û^ Ì?c7`x=Žä?§¤Y«¶àN?'_•WÊÏ?ì•ÖÍÆ`¼?²úcÀ¼»?"3ÜIA:|?~Ñ-sÇ?¸ÊÎôæÓ?² §ÛÊÃ=?îì+lä1?¢Ùs²Öá·?w'°Â?$?LÈ?œ•æz«"Y?Ÿ«&RÝÅ?ëHÄ÷¸«$?®¨Anna?FVìïÚ?…‹#º8X^?ÀÛW‰ò?­,b=õŸx?ëFSß%>ÿ? 0t¨£W?"SÑQÐ[?'¼[½w?À|6bνy?¾J–
ʳAGN4FGL J0406.2+0639¿ç—oRÂ&À@Ô^'…ÏÀ:£Àd¾À;ÿt²G@{Â4moð@l¬#	"?ÓYùñs¿'ѯà'â?ÐDƒEW@ž0ªlЎ¿ÍÑð£Ä7¿ê1[Xo®¿ëñ±¾SF¿Þ—\R'G¿âŒœÆtÃ÷¿Û|c=gµUNASNone?ïv¹¼"ˆw?Ýxٕ?Zïáô¿­?VºY†oÍn?Žó˜co®<?‹øIÛÉÈi?ï›bßÅV?"©è?Yê퍤P?_3¥s•lš?†J×EŸè?'e
@Em…?í{B~j?£*Œ¨fÞS?vp•BŠ§®?rÐ÷ñ•?²¾æÊæ^?¢Äî½Ï£?ï.
v'Š¬?t<6Vô‰?Lˆ\½Ò6ì?2}î™,?™ZCƒ›'?sÝ|(ű?îQ­ú?¥V¹íX%?uЄ…<í«?p¾¥>SÒÚ?¨-ô t€æ?¤=Æóºm?îîr|^?¢rR)ƒâ?c&zOŒ•?pÂÆo­»N?ŸÌá8¢Zt?¡Î¯¾Þf?êj5Ca\D?²´¬¦ñÙ½?…¹¡²þ֛?€aKd¤dº?ÄûÖ7ÀÈ?²IB™´k?íD±¦3c?"§¸[Ú?i:+ò»?Wú2	·>¾?µª¼'À?"°;WÖÿAGN4FGL J0407.7-5702¿ç*`og¨ÀF4¯O
"MÀ;/øIRYiÀ<ºª¤ƒØg@'šúlÃ"@Ù{f¨«…?¾/p[áÇ¿¹‹ä$WM?ûúÃ.¾Y@[ŠPÑSÅ?í=™Þ¸Ý'¿åÉ>ÃNŸ¿æ:V=#vþ¿èw²ß:みæ­ Ε?¡>S‰ÈUNASNone?ïЍq˧ç?'‰4՘w?BRÆw2?K²(g{?uoÂo?']è¤@R?ï}£–‰e?‰F¦?ŠÓ…?hGÄP+°k?q¶)>(?Š…)iº®?ƒ1Þ4ÙD?讀"ýd?ŽÊOÐêí?l^ßÂÉlß?m'ÁýÅú?™ÿp²zî?rt'¢TS?ÄÙR0?i6SºÛ?`çۂ-}x?JG•ñnJ?…cWîG~–?g¦¡júnù?ïyÌHŒÙ?'Š÷n?`D,X¥=?^üJi1Ô-?{÷f6<h?Y&ÿ÷†/?î¿eb§·a? Ï(|ý«?uÑ"âc?"°4¬(>B?¡iµ•þ£?›©¹ã–0ç?î;'K¦û
?™Ç½Ü!Œ?z¸;!ê»?uàÜ$8Y?¨ö‹f(?˜ùÀ9°>»?îaT>y@?ŽìÓ6I?€ü·ÂÐb?s——Ž,?¥«Ž$¸æ?Œ·;SÕtAGN4FGL J0409.2+2542?íõ½B¯ì±À2à}=B€®À:ÁZˆâ'1À<T3\MÞ°@ x×­{xÇ@#!m8?ƈï-ö?°'ö¸»F?ì2C¬ýú@7;«|Æ?ïï"'`í׿çä‡v¿Ôƒá6]E¿ÓØ-=¥Òã¿æ´Ã { Š¿àPÂFbUNASNone?ï¬:-x^6?œ4®ޕE?F¡{¾íH?Z"½}M*z?ƒ‡\çGÞw?šïÕPÚ!?ï­éª©}?~û["T?Wºˆª›ý?\·"p€Á¿?ŽDFA?{ùîÝ;?ïbJÌø?}‹@#%[?a#,ZÉö"?Wœ³²ý÷E?''JOAw=?{ŒÔl"߸?îŒÕ»UM‡?~2¥ bÚk?t¨¹Üö?TJ¬~ã?¤¡H x?}`¤-æÙ?ïiL¦»"ë? 7<p2gè?V£Eyº¶µ?hLO¾¡e?'l6ɐŽJ?ÿç픷j?ï)©àÊÁÁ?–Ú(ÏçN?g¾/C,¡?s?¬è|½Ø?—ÒþvH?•@'Ù\?î•iµ6"M?"ž¾¿"?l`?˜Ôy?f®+9ªG?¤ã`±ø^l?'oGüè?ëì0D7߸?–ïs|	Ìï?ŠS),P^?s¥Æ˜<6¼?½TµGcÜ?–Ý£2gPAGN4FGL J0409.4-3822¿çÚ½/ÐÀG´éNã'âÀ;
Vƶ2WÀ<D@¡±@ ©"- Ê{?ú~e`¬é?Ó듡ÝàÆ?ÜÈ?xæò@*Ï1+7@ŸPW±A׿å P!Öi"¿î؞ý†¨ü¿°‰%BûR¿ÇìÎ_tÞ¿åg쮤"¿å%Ü2›UNASNone?ïÄX ÊÈ2?mUP•tëí?QKÖÊ©ëL?FƒØÀ&G?y€ùÞR"%?jþaæîÕ?ïNý`hv?'HZ\£â ?rz_¼YO?vaÞ,Ã?'¡eä':?Œàä迟ý?îà4ï(Ÿå?'­ëÇJ.?yäisÑ{æ?{œ¢Ü×è?€Gº´n?@Dž
!‰?ìÜӐÑ@?))§Àº?zQL%­ñŽ?baò¿Üj?·tO@nªå?}Îçùâ?ï†ÇRmÜ?'Œ¬É¾¥?f4—¡CÊl?auͶ{'z?ˆÁzZ'‡?€"ݲšÕ?î,
½ü­ï?«kæ²?òx?ƒºÕSé?'4?"îÎ¥?¨PžÙŽ?¦Ëá ‰ó?íÜí¿
ÂQ? Ý,¯¡?~¤?~TÓ",?®\¢Š‡l–?Ÿ·äv›?çöë4Ó«?§Ë)ؘ<_?ˆoP5p¦æ?z¡Dƒž¢Æ?Ν^'ܦ?§Ž
›CÑAGN4FGL J0409.7+4006c¿Õ¡,Ãàó~À úG²À:'OÐ"À;¦y3Ȅ@ô¾}ÿŠ9@)YE³Æ?Ór½â¤$?滄Üޓ@µŠáoò@02…8cŸ?ïìv`Y‡?¢Â{÷-…¿èòF+]|¿î3¡˜@©¿ïü´%t¿ï¯žŒØÁUNASNone ?áœEL#e?ÈcTt\¯j?Ń3¨ÆT°?¿¨Ç}
Jd?Òۓ±oœ?ÅñmøÎTÚ?Ҟ¸TFœ?ÈRI'o?Î		³ª?Ä~çO¶$?Þ\Ÿiߏ?Ç<à׬àÚ?áïɳà@?³œúˆ¨‹?Ävч`v?­9E'&q•?Ò±/|3F?¯•÷
©u\?Ñ"þÕ2¢?¢ÂöÈj>?ÜòÙÚZ?«ƒ+ù@
Û?Òáx'PsW?¦ú…iLO?Übæ'Ää?Ɂë®[À?ÍJŒ0?ÃFèë‰?Ôø‰Pm£?È	ã+'†Ù?À¤š£ÀŸ?Á—Ü
‹›?֏dÙ&D?Ì<0ù®=|?à'HKü¶?ËÓ¼ç7ÃL?ÕÃ"´?³Ú{|œ5?ÎAiú ?´ÂL…¢‹?Û9RÆeCj?³Üù²âT™?²dï",6?"º§ _?â9€AS²?µùø~"K?ÖóÃ[®?´w³A•´xMIXED4FGL J0412.5+6519c¿ê".˜Nú@$c€ÞôÀ:÷e&ËFÀ;ˆ`¾†¸ì@u3Ú¢ù?@±z`ï.?ÕJ*7!?ì~kàùª{@	ÃJ¢»K?ül¶-‡£?ïô´<³¶¿ÑÀa"V¿ìœU•:¿éEV¶ÅúK¿ÞgÜó‹}w¿ðUNASNone ?Ù»š'¢ÿ?Éö¼pšX?Ã,Gó¶¾?Ã%,jIC?Ü®Boށ¢?Êä8àWT?ä%¥Ä½?Ðõï¹i?Ȋœø/n?Ç9
Aô¬?ÆáXpÀ˜?ûG^²?áMÚQïü?²«w??ÃVÚ*6?¬É+ýeÅ!?Ó¸Þ¼Aÿ?°ö‰ˆb6A?ÓÒ¶ïsss?¯~Ù1È?Ô+ý¥Ãڜ?¶X‰ëçõ;?ØKjȱñ?°N¢™UM¦?Õ_ÉCo?Çàˆá~=?ÑciڗÄ5?Éð1£2–ø?Ù={\Rø\?Êiiµ85?Óß=f¬¡"?Ðï÷øR?F?Ü,{œa'Á?Ñó(2Æs9?Ïèùän:?Çǽ›xä:?ܯ7L?³*_~?͇úñßg?³¿7-;ð?Õl8ù×Ù?±úýxñkX?³–ýׂ‡? ùŠ­Þï?ÞoP÷$ Z?þPä…6q?ܪï§î&?ÁEFl\0MIXED4FGL J0413.1-0304?èÃù]ñÅÀB'žùTëÀ:7]à…ç5À<$'sZj°@‹¾‹–v¤@óæfÑÆ?À·©°=?–"ÆÜüMw?Ò¨~oǎ@8™E5ê?ïê
*%mx¿áçKh´€¿ãåþAcøx¿êkGa=‡ ¿ëQƜ1$¿ïÚúWI'ñUNASNone?ïª$—ˈ?xøM¡£õ,?`6œ†ÍPä?XšC?i2ù›o¯?vbXÿrz?ïœ	©žN?²K¬zÁ˜?]M-Ö'?_Ñ©pžC
?…ZìN?z³O­Ò2«?îéÈü¼1R?ŽÆ!²¹B…?€0NgÇ-‰?~Û	ˆUZ?š®¹8Úÿ?ˆD´¤‡À?ï6ísF¯Î?r¢O`'?xÎŒ+4s?\—{b H?'îÌ76ß ?meE>Ë?Ç!?™ñÛ[">?|õ¸ÎǕ?y](ø6Oû? ¸8ƒ8µý?—¥='°ìò?î՜<I	?™ÌÃEB2?p£lôýoæ?wÌÃÒz#C? '΢yŒë?–¬‡)vé8?í5CióJ?ŸÉÎWËÊÂ?"•ÆȞ6Y?Þ l™Ê?¬áÈe°4?˜Ñ'>L/È?íñ[¹}ÿN?Œú"—g‰S?}‹€ƒt?yʵ•€‰Ã?¨«~©–Kb?‡Ü<¶§ŒðAGN4FGL J0413.4-8609¿ÞÃÚ/"À=ˆ]…TÖÀ:ԄÁ›@cÀ<yþ+êi–@U£žU@?ý«>݋a?ԉ¢Á
¡Å?äϺRvÅY@‹ðÜvü@m÷[ÐL?ïüWÔÓ+Œ¿ÉG ½û"Ì¿ÝôÝ5¿è£˜ Õú¿ëJ9ßö¿ïøŸ^›—UNASNone?íçfá¶hÝ?»
vóɳ4?£vŠ6?»eñêq+?œ&óŽ÷aó?''ì"ëvã?î| ªoÀ?µvf[ /?Ž+(ԈΈ?‹"Í§h? ³+%ža?"Äì€1û?î˜@9g;?™L:C²W7?—–£ß²qq?f*‹,-?¢‹*$"?'Ӂŧ?ì|'ÓŠ^Ç?'ò.Õ,L!?›/eˆ,û?~0¾t©yþ?µO¥IÝ?Ž§tŽŒ?ìçÝp¢Ä)?´öQB¢Bß?¢m»û[e?³Þ/g¯?¯lûT?_? ØE-'¨?ëƑ
ÑFQ?¸ž®)¿.?£'t‡8'?¨õó€£{?¸
=O'™¸?±u£ÿ7Óã?ìI¨MšQ?¤Ä͟¼˜?¤»2¢ê?–r,ˆÃ4R?³U$'L†?žØµà¸l7?è‰(P^ż?¨
MØó–?¤¦í9/Ê¿?'Éc¨õ@Ú?ȱ£pÝã ?¦º[ÝAGN4FGL J0414.3+4522?ÝÈ
lÇvÀVn¡žJÙÀ:ð Â'ÆïÀ<4؇3@!I&uà'?ÿëÕ:Y˜?ÈB4‰´t?:9$A†? HŠ]f@'ݳ$A¿ïþ؝»gJ?Ýy¤{õľ?ïßd™¿æÒ®Žd•¿ß^Ù¿¤p7¿äq`Ëò¥UNASNone?íž:¼z«S?¥¶*ðÀ'?Z%'¡XÛÞ?M4ƒ
'?²¥"ÐÔY¹?¥{ŠþµÍä?êW1!,—Û?Á™š¦	¥?\»üm=ãî?jTsF$?ÆiÁä5
?Áp³Fá!?íLªŽÅ'U?œ)©ë£?yM¬'Žó+?pÿ'­Sk%?´ÐÀ]Žã?›&þPæ=?îM6ǒPO?Ššh¦¦€.?cÃQžb<?Y¸ÄÍ
??©ð^mæ»Ë?‰üyQ"a?éÓÔhw«?¶öÛÉ¿Ò?j:ˍô~#?]O=íz-?ÈGÃ/Œû?¶Í=Døæ-?ägsד$?ËýÙñ3Æ?du…Î@¬L?|Bð:É(J?׶Fª0?Êèäk{?éOâñÜV?¬\Ûú–&?‡­=î֕?xßeÊïÛÐ?ÉE ]®
?«¨,Q¿%Ê?ì*Yþ¬¡g?¤Ó¬×7T˜?q"@ûHT?r,Öi¯ú5?½"ëù§?¤Œý¬xuAGN4FGL J0414.6+5711¿ïgà‰©]@͖ hÀ:nìzçý«À<!¬%XC@ á "_Ps?ÿN-E	?ÇoØ‡Àÿ?¹ÝtÉâ?óîZ¼8¨@gք±€?ï¥]S˜.¿Þ#uP5¿ß¥I»ŠÛ¿Ü("Œ,ô¿Ølª'õé&¿êkó™mûUNASNone?ëqÞÖíí?»>ÕNc?iò;_Cá?bÞ3DډQ?Áм'åAÛ?ºäcŠq'?ç[¢VñB?¾×$ÃȆ?†¼€~‰€™?‰;ßc?Ñ3d·ËÄö?½ØóæðB?íˆñ•öö?™´¢¡Ž&?uÎü L­­?fGä~òß¾?²[ƒ‹õû?˜øSä-¼|?í)#ËóDA?®°XØP?z◹île?]Tw<«¹£?µ¸$8r?®|kÏ6?åsÑLÓ?Áïš{°"L?z0"'Û?kµ T$—©?ÕožUbs?ÁÓäѨn?ފÁ2‡å?Ä[CnOúû?Oֈá†/?"ªm#l?àE`ì2Õ?Ä'ƒdgÍ?èÛ\2–x?¬XÕÁ(ƒ÷?ˆSZEç7?xZϧn(³?Ë
ZAÑð?«©/ÇjxŸ?çâÓ£šh:?¥›A@ek'?Ê8Sö¥£?|ŸŸØ£öº?Î[jg…}á?¦ùö,•ÖMIXED4FGL J0414.7-4300¿î¸A롓ÀGVìÔªÀ:Ô qúïÀ=Û4nœ–@ÿ
Nãgï@Ü¡Ü^:H?ÆÒv‰Ê?"a(å@I0¾
í)?÷I6W™ƒh¢"K§¿ ¨áž)¿Ýýj#ŠHÄ¿ì"PŸTÄ}¿ïþ‰]aZ
¿îÌhÞæªÄUNASNone?ǜÚzÏï?Ĭ¥¡ ?ä\DÏgÝ?Ëä«õ«'?Çý´qóHž?'hÁ#e?²^G5®¢?¸mêM|?ꝯ_Bt‰?À>"š´¡³?¸´=Ñö?´ú; æ ?Φ괃½?°sþÀ=\?âÇ=R;?³»²(ö]?É9øXZ£Ô?¯ûµÏØ?­vç4üR?". ý;)¢?ì©õH…Ä"?Ÿ {ªÙ"•?§éÃ÷'Ój?•EŸ[lt?ÁMn±@'?ÀôJ:òÖ]?åœÔ®åÓ?ÌøqžÜW?Ê ü.( ?ÄÙ!<Õb?¨Á~gž{ª?µOsx?ë'ö?Â`×­¶?ºÞ¨4š™ý?º(ÇÆ
üÿ?ÂØ—Ç?¨zk>V?äˆMZŒû?µ ¡Ç?ː³þ?³"@÷µç?…-3,Óq?vÔg¯<r:?îNasÀ?]-ݧÉ/?¥Îœi;Í?šÑ«î"™PSR4FGL J0418.4-4342¿éb>Kj6«ÀF¿á2µ^òÀ;ÑÅ6ÖUãÀ<îì$·o@"-¡À»¡?ödc§oE2?áw¿ßÔft?ɼŸV?ë~X€I¼b@¹@œÓ4ñ?äÎô?¿ïÿêÁf½?ïûÞ.ôà¿àòF¿2/¿ï1½è-{c?î2þ…°UNASNone?î½þøËr?¾<Ö¤UÏ?k:Ô(Â2?''a4F…U?¢lqüÉI?»Tß!Ûi?©j`á?Žüê½Fɝ?`FˆS¹Ï?i˜­i"ø?†Š³'6?‹•8»ý)ˆ?íYᚆ æ?£<^«)?t…Íyvã?yÐZC?³è¢ðt5¡?¢èÏEy¼?î¨8æ¦g³?Œ.É6Ø=Ë?Iu~ïƒÛ?C!•_gMî?¥›–×™ñ?‹ãÞšó?îH› «:?´»ry/›î?rNû9‡?‰_œÑ:"?©5¤"oÒ²?²óQ-r"–?ï
ÁÅ»>8?žØN¯<Mv?gC™Øç¶Ö?xù|[l?›¿Tâü-?›Ùõg;Fª?í*ÚÆ×â¢?£"ž[^ñ?wi©ő½?~]/¬{(¬?µ29sÓ?¢¤,Økµ‡?ì`ù0TW?©DÕ ¹|?JʟӸD]?Zݧ#é"Ö?¼Â¡BãÝé?©=d7¨¡AGN4FGL J0418.9+6636¿ï ZS¹Þ@'¬%XÀ9kÃA2Ð7À<
òPŠ@Q˜âdŽ ?þg:×lc?ºØ6bg©?ظ¤¡µqç@!ŸØ­«ŸV?ûò§b,
?ïÿ`Úá8¿Íù/Lñ ¿Ô9-H7§¿áß¡@,¿íz4y"P\¿ðUNASNone3FGL J0419.1+6636?‡YdÍCb?Š"d…Âu|?îcø~ñ"?ª1C,ÆÂ?£ê§ñ?¦FúŖh0?•øœ).*?œp¦áI¿?ì‰ôú­?¸{àpú†G?¹ý‰O–ã~?·KXÎ5H/?œM ó8ü?"Í5^xߤ?鯹\
J?¯ ¥Ö­
?Å·vrçÂá?­ßšëåR?²oŸrò?'Tb"¡úî?çEÛ· h?¥âÄ7«Q£?É´
¾¦?¢Y½Ciw˜?¸ï·f?§Q©pR?íÕF:n]M?°¬£W?«={Þä¦?«ÊÂ"Ó(?ŽèGOëgÒ?ž[r^ŜÓ?ì.Ý*"?½¢*¦‹‰O?º²à/³ªp?»|ë3ÑNù?ÿÜQv«ˆ?‹ç!‹
͞?ê¬|c—™?°´HP¨†?Ã/ƃÔج?¯ÎHý
Ì
?—ù'ÙÖA?~óõАŒ?çÝ Œ3÷Ì?«ù¦šjM?͌XÓÖ¬J?ªqDdYPSR4FGL J0423.0-0943¿ïþòÐÜ?ËÀB¨'_ét£À:ûPÍwíwÀ<¿:4¯46@h÷9±?ÿþó…õ?Í\i¢Ûâ"?Þït—'e@ŸÜœM©@ˆë؀µ?è-'	'`?»`̞¿Õº˜b¬¿âuÛ³¿íZ·qõO¿ïùì?®ÁŸUNASNone?æiVÌ-?Èû·*?Ã賁è3?¼6ϽöxË?Âqñ·	cx?Æ»''ri?í'rQÎv=?¯7y<­?¢€2.²? '©M|ò?«¨Òéé¶?¤eÝLÉG·?ç=Þ«
t?³"­Oó¢?ǦõÏÇËS?°¨G2HÆ{?¶Éåjª";?¡Ã¾?ÈN?ìœmôÐ!?'!ٞ¶G?§9ûêÀª_?…*Ê='?Ö?¯=8†Œ?ˆ0°
Å?ã¸N_"i%?ÅĬ—Î?ÍcÓ¥ë?À_%ٝ."?ûıö1Ë?ÀEà6-…í?é;XþkLÍ?Á@£ý(gÜ?¶´…PöãX?¸ßF°IM?¿p²¸­
È?³$è^üú7?áÁ÷±gì?»lí?W?Ôº"í‡z?¹±È¤ôì|?¿ÌcV¢µ?¥üø1×ð?çÏWº@V?¦"~>¦,E?¸À)_ù÷?Q%fµÏW?ÄbŒ‹­âk?¡AZ}Ïä"AGN4FGL J0426.5+5434?ïã®uÉ°¹@ûH
[À8VĘJåÀ;(&Ú@èÛ2k71@"÷Ãñ[ø?­€4¡Oùñ?Ùô/|ÅM}@$ãBؤ@ÿ:)Â?ÉÍ8¤û¿×ÄaÄ@6Q¿çÍù½ÆŸŒ¿í¦Á Hà¿ïü¨'Zà÷¿ì´¿ÍhUNASNone3FGL J0426.7+5437?'"ÌX¼7\?'@tµY?ìn"Ç>\K?µ•»²?¸&æ°LQ?³¸õ#?£X"ÝÅ?¹»aþ=V?éïÐ.Îl?¾<öf?Ãyé<¼kM?¾ÿ{Ã?Ä¥¶.6…?­jÜ¡8ñÏ?å쫱Á{?´<6"e?ç›
Äu?«±šØŽ?œŽP£ƒ?€¡"˜¥?écè
˜Ë?¢Rn¾¢Þ)?ÆïN
÷[ä? óËÃ|/ë?',ú´ç}Ó?'¿t3Sv?ëþ§ZU?·‡zóÿ%@?»"$9k?µ¸xÛµ¨+?"¯S\vã?±Mºuh?éõL¢…?ÆÛ-ù›Å?ŵôaCðM?Äå°¸2ûš?¿fù¯êúñ?«L·°uì?æqÓ{op?·_ºtIlÊ?ƅ5:ÄÇ?±¥,~á¬?y÷ï^sÞ?c%'èÊ{±?êxWqân?¦úéÔe4?ÅNâÀmݘ?¦‡^¡©'PSR4FGL J0427.3+0504?ו5Uf'ÁÀ<ÁR*o?SÀ9hŒs@À;¹ðŠA7@X'ßB@°†£Ð?×9''¦¹?Ã'ǁ&?þ*9ªE¹H@
j»q/ÿÅ
x¹z4¤¿æia#pÈ¿éÆ3k	¿í\¡V&}B¿ïÿ2 ;IW?çZòʍWlUNASNone3FGL J0426.6+0459?ïòŠÏ¯Þ³?ZòôPÎ?/Ü'îdÊ?9x?åŒÁ?Vîۜö©Á?Uó!š	y!?ïºÍìåúy?š>²{¾k?Uë`©÷'?ckŠwÈ¥?}A˅±§?}°P+L?ï.{d¿2?ŽˆndfÐÒ?r9mhôð1?vý:Fl0?•¢8Í°?‹³7þbá?ﯬŽúëT?eV•©Cá?Ye–ýÍ?AY· 1?€è,GÞEX?cqIG2v?ïâãÝï¤?m´Nˆo–ä?=ÎåàóM??œyE<aú?ic:͇c?k¹V—I.Þ?ïQÑ©_?¢.À5NfL?l†¼ƒ¿?~28šyá?™DîTXˆ2? |ÖûÃ?î¤UÄÏõ™?–˧|¾é÷?~JUµ{cÚ?€W˜ŒæK?¡ñXûÍHü?" ÞZ´n—?ïž ƒ,?…tˆÖmu?r"BQ:-™?bõ°ç®x?™gr@G?ƒ
3º^Œ†AGN4FGL J0427.4+6433c?äê×ä@%'"ÂqÿøÀ:.®ZZÀ;¾@=ñŒ@ìýåžÝ@[yJ]?μ~`ƒ"Š?ÓÄ\:é`@nò[Ҏ®@_îZ;4ß?îA²¢i¿…¨ÛD\7¿çžÖà!t¿ïaMl·ä?«Ò¨²FÓ¿ïÿŒ!áÒUNASNone(?ìôHÚÂâF?¶</cÎd/?"'¯,X—?‰6ˀTK?µËƒCéO??µ" Ñ\?ì‰CŒ¶v
?¼T³'ñ.?"MѤ_á¶?šéëp´`?¶¢o0Æc«?¸ÍQÜ;E?é'W|?ª™Çޒ?¯õ6a	1?žû¡ÇF˜?Ãeb¸ålß?¥[/(F! ?íÁžm5Yö?"pŒsÛ?9è:-Ñ´?sB7Z¦¾í?¯—ŸÕ¯?'?´õeõ?éÕÅ@*VZ?ÀtŸÔ#â?¢Õ'++Ëâ?¥a
†_œ?Ãó†tù§ ?½#?þ¦AP?èW@*s\?ÈÂû½¦P?®R˜Ü¸Û²?´ÒAi?ÇY Ïû£?Å!‹5RÈ$?ã탛Lïi?±y~1 mæ?ÀÝ¥‰ÿ·?¨îý=Ù?ÏlL'BB£?­?+^"«?é&,°ÉGB?¯ ÛÄ"d?š6DéÀƒ?"Œ"	U™?È "ž¤Š'?­$ÒlOݯAGN4FGL J0427.9+3632c?ç²sé}À û`'ŸÀ9'É"\h·À;mθ_W@­ÔI@²U'þ?ȾfØ|-x?×pZ›ü@‡è|U»ô@q1¼'?ïÛʖ'¿Ü‹}At>–¿és"ý}™´¿è‰ŠøìæH¿ïèí"Ãq¿ïé¿KÚÉæUNASNone ?Øs°¯hl?ÂUO6b×T?¨%™ŸQS*?†â‡ÊW?â|l¥x(?ÂvOùCx?ÝIñ;Ó&?È뇀›?À÷^àyìš?´ãZ[Tà8?Ú:_Sïã ?Æú.My?â,~Àœµ$?²¸¸q‹?´–Ãï'D?œ…ø/Kÿ?ց{΋…?±Íçqä
?âYD|îœ?¢¤Ömó>?Ä-M*«$[?˜4gs~=M?Ñ6ÑQ°›?¡_–TÊðo?ƒʃ­…E?¶Îñ(r?¥ cÏg™³?Ÿ)V‡?é	G"9¡ó?¹9¥k0ò?ΎìRµ?Ï?ÅLfDðº?ÍÙ¯˜MX?ÃFZâú‹¢?àåÙ?Z?ˑïý.?Øe4…¡GÁ?³OÃ&yÊ?¹ÜÆ:ȏ?¢ÖÙS«?à'ÌõÖJ>?³¢üõ?¤ß?Ó*'ÏZy?£XNªðÊ|?Ñ'°PÈÍí?©œ×3$'ý?ÛÉ%‡gי?­}A¤yÂMIXED4FGL J0433.0+1327?ãùÙ©îÀ+À6©¦
EbáÀ;8×ôH;ÙÀ<튯@ÎpþDéê?ÿÞ5Ìj§?ÓiÎEêœ?ïÿwåëo@Ìã=Qš'@@¤‹¿êÒ2g[Y¿ïénù²Þå?ï½è=–Žw¿×Àó°fe¿ïÌ&´Ÿ¯]¿ïïNÒöUNASNone?㷁R6ó?Ɨ¶ñÕV?Ó|û~?żPÕc?²‰qHx±ñ?©çÝK)†þ?äѦÙÑ¡?ÎÑÅF½öè?Ѿ›ÛW?Í<­Zk±?¸_tW0až?³ƒßÜ?á;äc±,?µm"µ+–?ÒæÓ20m ?³@»¯v®?ÅBÈÚÀ?«×=^ÈG?æ³*¢žƒ—?²õÔ!/?ÇśÉ'Yi?²V;®s?ºÛsX½0x?¢¯¤¶ÂÅ?ß©
™µb?Å"I¥DÈ?׉àL)?ÅÞX‡Íá—?Áš$4xé²?¸R·ü¾Ô?ÛášNË?.?Ѩoí›ð?ÛEýV=µ~?Ò
F£ík?Á°Ðµî§?»^—q:Å?Ø{7¸lÝ=?¶•|»}Ê$?Øà÷Ïk?¶~©ò4îÓ?ÍIbŸ‡oK?²ãæj"ØÌ?ÚlÅMÁC?Á<iÄ%¦?ז…7·Ò??Ä–3ï¬Ý?ËúÌôØý?·½áKªMIXED4FGL J0435.5+3232?²Ù-0a]À$
ƒ{á"À:ºÁ濽À<P[¡çEõ@.v‡›À:?þÑטةz?̍ø%ÁÃ?ØèÒý='í@	ñ9þÿO@õõ•måâ?ìÀäbÈ?íúVrÓ\3¿'Š FJÖؿމlLþ¿êz:Ä!, ¿ï"ž"?pUNASNone?äšDB?ÅMQÍ':¬?´À
(½?®¾ˆ=Y?җՁÄ.?Â	|«w<¢?ã¢/üƒ?È==²+ûu?­6kš)wÎ?ªëÛ'Oò?Ö?íŠvTà?ÆÛF?Ýï?ë6dÜߥ©?¨.üÙå!?¨1Â?·?—°$å+')?ºJ@7u°?¢å㖊<ý?è;ðBa"2? %÷¾Ž'?¸™l3#Ð?–AÅ©4DÀ?ÂÈðïO?—궕ô`Ÿ?ÝÔôÑ0Ð?ÄÖkқ:?À‰ÀúlÔP?´=dt?@?Ùæ*±¯e?Âóu«ÜDí?ÛIËPý÷?ËU­à(?¹V~^º&€?¸CŸpú"?Þ`•LõI?Ëqò€æo`?çæ¦ñ#¢?²8º"³ò?´Fˆ¿¦î?¢º gy?Éy!\¤¤B?®ƒ_	i¤ù?â¢'!çB?¯±¤'ë?Ãmÿ7¿E?©ÄWÁߓ6?Ò2Ü QÚ?«GÞSòkNMIXED4FGL J0436.9+2915?ԖY@Á™ÆÀ'äAVâdåÀ9ÐϟåãõÀ;wˆ4íG—@3·EQö@Œ²`9ü{?ÁçZS<=?ÎbZû¤&@ú¹o!÷?ðŒ+$U?Öº'#'à¿à·n=h¿ã|¨Ý"U¿áüî
ö¿îLb-<¤¿Ø1Æáü3îUNASNone?ÕB;@jJÄ?ijÙK?¶‡Jñó?¬¤5ûu½Ø?➁neÊp?Æ
SC¹?㛎ÙC 
?Îô@?qk8?ÅxŠÈà?ÂÞTýí?ÌC(Ÿº?Åè	3…hŠ?â}å÷R1?±Â¦ڈ,?¸>B¼¤?¢|Gô]–?Ôô¥Iâ2v?°Q£$3›K?е@_|În?¡âQõ9T??Ènš÷—É?ž'¡H~bË?ቹN²×?¦¥Äot?ÉHTpÃ.?¾Õw¼á-"?ÉÉÿ#Gi?¼MÓä̦?ã;kQôó?Å oC&<Í?Ø™"ÿ·?ÏÕ|>Ò?Ôª'C«j@?Í=8š¦4?Ó@ä'B J?Ê¡Ê"aé?Øò
^Ûû?³cs#m€R?Â"¡#ÀhT?¨u€~£E«?Ýü¥hÀïÛ?³¡L?·ˆÕï8Ç?•orY—?ϛÂi­ª?«ò£FÒ³}?å'‡´ÐèÌ?¯¶â3I*,MIXED4FGL J0438.0-7329¿ïŸ
Vg$ÀA—ŠC»@³À:n¢‰,dÀ<}ƒêXÏ@ ¦'æQ?üADˆÆ¿?ÁÅøâG]?´P°Çˆ•:?ó°¹÷2ú@¤h$V¡w¿Ü½ò%Kê¿ìI‰¡Sø%?¢GŸë‡¿ÙàP7Oøf¿ß\*Ãx[¿ßd3›¸Ø¤UNASNone3FGL J0437.7-7330?ïÙ÷é00?eJž"W%P?9y"S¨¦?(æŹVÊG?qä<,J7?dŠaᨈ?ï®û3E/h?•pāƒ?PéØ£©¸?UÔe@û3š?'#øg­Ç?€
€õrƒ6?ïm±âˆ?{‡Ú ꨢ?Yàè—=Õ?MÙ\	.âÃ?«ÜsP21?{½:¿ä?ïñègT?s¾~fövÅ?\4bì2–?AAëSEÛ?œdC—Ÿu?sb$á|Ò?ï­Pò¥"<?xó;̶ÞÃ?P$·h[?DUi£†ÊY?'©þܶo(?wÔljÝ?ïXªˆv©?œÎ°=$A·?_ÍÄZ>»)?j©´ÈŠÏþ?œp"m%?›y(²g ?îÕ'•¥?€ìÀb[?dVSà±ý?^èyUËFa?¡h);"?Œëâí_9?í|CFjŒU?'¯—'\W?n_:\L#?]Ab?¢À?³*ëû€?'fíAXÝ3AGN4FGL J0438.2-4243¿ä#äß>ÀDø¿p]À:¾Ú`3FÀ<Lð\@D&äpX@g ã¥Vf?Á"žy_g¿®	§ô{<Œ?í®"áÉ´@¸"ŒòÂ*?äYo<νh¿ê$DîFš¿æM™{f¨¬¿ê—v©ªˆÕ?γŠ›úÇÝ¿ïÿæ4|ßOUNASNone?ï¤ÌùîC?ƒ`¿ )y?[Á)±Rì?] LÌms¤?ƒê'%šÕ?˜ºñ3¯?ï•8™Øx?‰EޜÞ¥?`£*Þñ'£?iãvÿ³ v?†‰˹–(?"Òx¶´­R?îëÅ:Ý ­?4f?ù4ø?r7Õ2Zû?vNG¼"IÈ?ùcW¬?ŒUl½ZØ?ïŸn>eÛ?l'ížg(j?7ó¬ry?-­ø§u?‡k¸¾U™B?kúpDCÐ\?î½ìÆè1? ¦"ýô$9?wkl{!‹?x¯×A?¡AS¥w&?žm—¨À¸s?ïš ]`·?žƜ"?fŽl
â?xž·ádP»?›ZÞxè"?š˜*8Ǖ?íÉ9žê*?›èIíï80?€Çq"<úâ?AŸ…Šy±?¯:"Yü…(?™×65°¶Î?îˆçð7¹?Èç1tc¢?XÄùÂïÁS?Vç×Í)f?¦«Y-Åjk?~Zô¤IyAGN4FGL J0439.6-8322?Ù²ó¥Ý'lÀ>•Ëeè'À;%Y>_· À<€RnM@"wïвà@ˆ:Ùð¡¾?Ó?Õ"[ʁ?ÇĕEÌé?ñ(º3m?üNøñ˜ß
?ï÷¿¾€^då¿ãY8œ(À¿âV•Ù¸é¿ï]]ÿ¾¿Ù>Ÿ¿ÎbUNASNone?ïRÉ!á@?‡‰·&ÜÞt?lrН2ö?d—B\ŸÍ?'¨¢{4?…@DD¦Ã¼?ï8Dç²ù‰?Ží¨nÜr?v"•/ÂZl?vç>áÚå?"n½·€ìA?‡#ð†KšC?î÷Í+—]?Ž"Ëá ?ƒ5´ij?tF"†?—z¿±'Í?…Å<;˜Ó
?íÊL8^t?ƒ5
Åt–?
å,o?n~N3¶?«Ũf?€ck?îÆZøt"?"
kBK£?y\ü
aÒU?o–QÝå›G? n°óäyù?'jWæ§?í±#Dí_?©ÊìbiV±?ŠÜXMLx¤?'dg°(×Y?®0׺Ùê?¥9³žA¼?îIiÞôu;?–2¹òœÃ"?ŒÑc&¦»?†Èÿ¸²c•?¤5	N·ž?'QBž"ð?ꄢfœÂ?œKåµs?ç£Ù1¶¼?‰¥g÷î¶?Â0êºˆ?šÃ{^Rî%AGN4FGL J0442.0-5432?áG5Ò'ˆÀD/§íåÀ:¸8!ïÀ<¨»5˓è@/ëï|Ð
@g­"ãY×?¼ï"ãñ¿­ëþì.¼×?ð:µ´)@v•]ŸÃT?åsú~
òͿ唐æl±¿çÝB 8š¿ç¶Šþøï¿ïÿpޏlð?ïýÕM¤ÎUNASNone?ïëJq›×??Y‹F™';õ?P§ºBÃ?H%eF¤J?XÃý"ž_z?S÷
Éq?ïGÿH)?½¸m¤,?^ëm$ZM5?c¶õ"©E?"Ð'‰lì6?|ã@Þٚ?ï_žâ€ð?[‹"‡áÕ?p‹Ÿ©+?r$A>SÚ?€ÛA5©?}Mí)U¡?ïΤ¡ÆŸó?Xé8ˆ ø?_3`ê {¾?G0Q¯¼wÈ?pàÖâ×Óu?S'¬_ûƒf?ïÍbS².¼?p*л}DÓ?h
9{ƒ"?bóÆ¡
¦?jŽžå›I?eàT¡'F?îòÞd#ëí?›gýÇðæ?m`Q^JmÌ?wûßCxÎé?ø)RüՓ?˜I>yt!?îéêíQ?‹©y›=?x!_¹2˜?xHü^÷<?œÔ*ºàØ?‡÷§šþQ?ïJÉ{ÎFc?~ˆ0o®î?}j
4Òâ¿?o»Äi4w°?Ž˜š|Sɽ?vÆùçsªdAGN4FGL J0442.8+3609¿ïÔ{uþE&À¤¡4˜ŽÀ9×äQMÐmÀ;ƒÔA5Tv@QBŸ@f1rhÓ(?ÆjEî÷š?Ño§BN¯@*F"bH@ªÆ>¾,¿ÉEø\Ȃæ¿ãß¤¬ó¿è€fAÓ_
¿í¤]­Z@¾¿çIžÚv.¿ïì‡b_p©UNASNone?é'?†A'ß?ºWœÒ'»?ƒô_^Œ?'lËNUJ ?Ê#»ñÞ)A?¹}z¼/º?ãneÃu­y?Òj'èFó?—¥0ñ?™Kãu"?×IÃþr`?³Ëù,!?çdÚ'ÜÆ?­š²A‡ê?¨_]bВ|?–Paô&§?Íڕ=ЁH?«ÌÀ _*?åiÂù†¶Š?£G×)þô@?¬fփç?‰?bÖì«?Ñ©í1Ϲo?¡¦y¥(0/?ßX¤Lâ?ÃvÊ)âÛ
?•â¿oš?ŒÇÓçéÌ?ßW-†Ôx›?ÃwQ+|ì¡?Ó<ó'î»›?ƯÔn¾?¯Gj~¢=?±®°Ð¬{*?äm?Ç^±ÚG?ÞAZ¤wO?³㔃gû?¶ÿê}ž? ÛÝ£ïê?Ü¥`æäj?²œ©†)å?ÖZ~§¶ùã?© ôŒiÈ?¼¹úL·¾ž?¡X
Âl?á;cûš?ªäȌ¹EãMIXED4FGL J0444.8-3514?Ô ×œÅ¯2ÀDçÝÊKÀ;k%ÈçdÿÀ<Ëå+hc—@sÆxIè¬@®'r—Í?Ð!DÚ$¤?°g3BE?Ü´_c@ý'öÛ?ïÞ43
s†¿ÙæFñV¿å"ÈA!ÞL¿ïýàÀõ~?ïàŸ°4¿ïñ$ЙàçUNASNone?ïåj''Ž?b{`ô¹‡??+äœV}?08'Ùšgf?hå
 4fÜ?aÔú›¬G?ï©H²»‡?ŠÞßCç?Z¿»&ê?k[^*ñ°Þ?'UÛÞFt"?†¨šõV‡5?îãfG:YÌ?EÄVòÛ?p t&[÷?r¬3'ˆAB?Ÿ‹	rmÑ?Ž±´¤)@?ïñª²?Jå˜S
µ>ûÑÞcþý>ýÛD»«­?\;šSá{?IÝ_€ Žâ?ïÉ#]äGú?tU-¨µŽh?@4?=§ÖÒ?yl
pkÚ?slâ¿Bï–?ï@ÐÙæ•?™ŸAfa9Õ?`¥«#CvÙ?s&´Œ—k?•Ñ/g^¤t?—£¼='?î$¬ÿkÊB?–\†]Ú0?~(?g[L?}ÙßÔ?Hœ?©ð(;±/?"Ç–Ç3.?ïÅÁp«ÂD?q¦òÎ? –×qËW?"ÝKˆm̚?|¶Å2Qqo?q†¼3eÐAGN4FGL J0445.7+1535?à[µ2|TÀ2ìUC(s½À:FE­‰:§À;·áñ÷ÿ€@ĆØ!@Yx"væ?Ó0p ¦ÿ?ÜBéŸ"w@	˅¤ð@ÐrùòŸÅ?Ѭ9d$­¿áËF¿Ä§¿èO¬½ã¿ï~µè"¹¿ïºú<q V¿è…™!y¢XUNASNone?í¸ŽpŠpv?®‡÷ÓÞ$h?†à*Ï@Ø?'ø);G‡´?®ò ëÉAq?¬‰qØZU©?íÆDÂý–?«A¾MNJ? Õg±,AÙ? Št†¼Q'?¢ÆLÖC ?¡¬ö4þy?éñE5¥d?«K;±he?¦È§7â¦p?•ôJÁπ¢?ˆÁ\M«&?§`à"¥Ÿÿ?æ¼Uðê?œjç†rc?³4ô_€®?‹@hîV	?Ëuh{®;?˜Ø7§½o?ëpZ
C?¹Cˆ0ÃÙ?—e"hä+I?'ï—Øfv?¾£Ê×Ì|'?·Ä";£¡?螉¡N?ÃièÑæA?ÀÍ,ZÉF¨?¿¥Æ×e?¹qZ<¢Í¿?³­ñKçr?å‡['璐?±¼ÜŠàR?´NÎ8?‰? ·ö˜K†~?Ï»*˜¯äµ?°-mv
?ÚG¿Ý%5?¦iW¢ø>Ë?ÁV~>Ü®?¤L–Á÷Æ?Ý=y!ìu?¨¬I]aÈMIXED4FGL J0447.2+2446?ïÿ:¨ûêÐÀ*]ÌcñAÀ:–8¦ÿ´À<LB‡ö@vWNñTÁ@æYeÌãs?Ò‹eNce?îÕëY€@~¿ù³?üµíbC—?ÙqÒàãG?ïÂQHÇïî¿ÐÕao0º¿êÕTáä·¿ïÿw¯d:?ïñ™À…ì"UNASNone?æy.ªÔ?Æ"c	î	?ãÁn8( Â?Ð|Ó+»¬?ÍSÍðÁÒ&?Ëa'AõT?Ôïår­hü?Íóg«µÐÝ?áÙÈkǬÛ?Í9‡­€N?½r&×õ:?»1Z|3"g?Ôt—ÆI"¸?²!1£È?Ý2_*T^É?³º'nŸHo?̲Äý?®
€"­$?ËöîÀ"Ö?¨Ë5¯«?äÆ>'?°õ½›|SÖ?Á•"ª&ã!?£½ûêÝè?¸U9ß0ô?»Ø"è@+û?æAdöh–[?ÌÄxé(€°?ÊÏÏ7؀×?Èc'ØDW?IJе˜0l?È­w:?ç · ô4x?Íß/p?½"¡'y~`?¿Ž3ù]ò?È^Û@
º¢?­3|_¾]?âTà-8·?·6›\¤\?ÎM¤
:ûÿ?²+.ú£Ñ?¯úBhê¬?–Ú
øȏ?耈ñ_º?³<p'=-H?ÅÿO'â–?°Tæ§ÜPSR4FGL J0448.3+2743¿ãÌ[°!À&TŸ"…^À:³jû÷]À;«Lg·Ÿ>@]EÌ=î@U8áÈÝT?Ï'öüK@?ҝû¾|Òä@*à~Zy@¿"Ë(²Ò?î–éP'¿Â"ž'¨'¿æ[™ï)îç¿êB­#º¿ìùYó'\´¿ïõø	'y:UNASNone?äs±ŠsƒR?ÂM¼÷AÀ?•Ëˆ(+"?‡C	Ü=?Õ»äh†…?ÁÏ¢+ÛÈ`?æí{~¯,?ĆxZ?£Ut#-û"?¡Ÿ€ý*2?Ït´ûÓS,?ÃDÞ«¶A?帍uÒr²?±KÁª.è ?«é¨Ê•ä#?—"ïÑÜœ?ѯûZÔ¸?°BesTéð?æõOEô'?žïLøc
?±vRx¬×?‡í)"JâX?Ëo™çƒm™?œ䍓?ܗL¶8Œ?Ä¢gq[ël?šM¹õ™E?ŽÊf$
ò?àä/'+û ?ĕCwè³¢?ßøƒ…—?]?˅üʈØ?¶{P#?¶`kk'?ڂ§ç?Ë|:߶¾?ß$zÉÂ#?³Æs"áÎÛ?·'aVé
#? Â'èˆ\^?Ú÷/Îq4?³¿-3?ݝá&öäÎ?¨Zm߬x?½þ÷þe{?œëTßyy?Úâ`Ùoٓ?¨Œ^Ž#ñVMIXED4FGL J0448.7-2116?êÓ»aÌúÀB€ýÁaÀ:wSeØ¡íÀ<láçDò@^¢›öÁ@‹Âßä?Å,ËåòÍ?Áǎ^ýçL?÷ÈÙm²‹@Y>:"e±?ï¢1þªÀ]¿â«¼|±¿è¢R_ô1k¿ãinX£/E¿ï½vþ«¿ïð­aÍzrUNASNone3FGL J0447.8-2119?ïó9 e®¹?J"vgHӎ?9ËÀ&È‡?1煗4V?SÎÌüÿb?EϒΥÒ?ïÛÚ:®?q?îØ
fQ??uÿ"ùž¬?K±BŒC&?pœŸM¯¬?n[	j$Ë?ïÄ/"
š?iaÅr‹?Uéy—à©?Vñ·ý¯±?xn~{N·?esx(Í×ù?ïÙ½"hi?NV5ÝÉ?Rñ
qt5Ù?5ÏSm'–É?lÉæKúƒ'?Iw˜Õ@vÀ?ïè'dÁ.?Z¼2ª¤?L
X¼ÊÕ?EKÞㄞu?`z˜QQZ?T¨67›
?ïŠ-~F	­?‹–}¸?Sõ
#M?dÓ¦6ž??‹¾Y?ˆ5â–áÏ?DÓ?seý¦W™Ï?[G'µÏH?Uáèq¢T?ƒ¬¸àC`?qZúHmC†?ïšà¨:µø?k^p-Ñ}Ã?h¨CKžTå?S¯¯6%…?ƒÅãªÂ?fÚc;v<4AGN4FGL J0453.3+2843¿åd_®™äÀ#
çöô¾ƒÀ:3á @è(À;¿p¨È@ÅXQzÆñ@%ن³U?ÈVãçp'?Ñ®äïÙAO@»Ò#Mââ@ðßP²ö¿Ñ=˜|c'î¿à£'÷Ó¿ämä£P¿éæg"N¢¿è4©TøÙ¿ïøT<jUNASNone?¢jW?¢VHGØ·?b'à,šü'?]]¨ÍÍ&‡?¦>§ÖTR@?¡à¨ç^VI?ë)kèA®‡?¼—®¡­S$?}S0ãìß?"O'¤Þo?Âo¸V•…Z?»ežïˆ¨I?íþ>EN?¡Ï¹Ø|¤?‰¥ŸI¨?'ãDŒç¤}?´S[øaÚ? i]a'Ñ?íh5™?‡ûsÇe(?z¶fKÞÛ?YÎAÞÉì?³õË՞0?†³
}Ã[?ëö{|£Á?³ÅªG-?rÈSb×0?n!+û0?¿žçóU?³i¥ç"t?æhõë:\?É,¤èqí?˜–~ H?›¨JW)A?Ò&<«¾"?ÈiŸQ¥ I?éÝdB'um?®1¢ñ(?–ÛO'¢´µ?‰ßÙ½ø¨Ü?ů¶¶?¬‡Ø'Õâ?è®ßK!?¢í¾çOé?'‡*¿è?x>9ÑNé?˝|ä=h?¢ S>Ñ²AGN4FGL J0455.9+6757¿º¦»¿o}@.NޗÐk¾À:ô§vÑîuÀ<·ö:"`L@ ‡y{ Ô?ù¦,ƒì‰?Ó#½¿"©@?à¸æÁ?¥Ý@€':O‡'?÷ۑنĀ?ïè;B¡:M¿íÊJ µ'-?³Ó6sXg¿ÓÏF0Š¿éBas7…¿ß?|žJ®UNASNone?í7Æ߇î?½èýÒJ²x?"á-pÀKN?'ø&¶°Ó2?³¥©|5'¥?ºÇ[—š*?镋UfÂ_?Âà،7u&?³j?!ɖq?±ÃZ9µ§?¿éf1Hˆ–?½^‰)4?í€3QÄ¡c? EH‡ÎØû?•ùºk¡8Ê?'±é æw?¬ÿíªu±s?šK²)46%?è(]•#è? RL^?Šá?µRÿ)I0?"ؘW>?ĵ
1Ð?˜ÅnâöT½?꥛ªËE?½çë1øܱ?š¼P΅¦Ì?––€G~"?Âoò'?¼ÈÎC"?âæ¯õ%±j?̖õV¸¸?Å! XKW?Ã/·H1?ÏD$îÿ?Ç9ËÕÎJž?뛝wA!€?¦óegã¿?ž¢éG®t°?"àԀ?»zYôyJU?£é"¬ës?àÑû®È¼?­¬ÈsÂ\–?¿~s¿|?¦½ '­Ød?Ö|'˜?¬ÝO˜Aö]AGN4FGL J0459.7-5413¿Ïn+
Â,ØÀBíZ[–(ÌÀ;Vµ–Ob>À<è،ôo©@û¾Ù6?þˆw'î\j?ÛCú*Óé!?¯9X';§ ?Ðú`ƒÎV?ùêmÿâÎÂ?ídÈÁû7™¿î;.¿±q¿™]©&¾8¿ËéÙøÚG¿á#[NÛ/f¿ïÿ%ålÖÃUNASNone?ïÜm»"?eVŒôیÁ?+[%ú•NÞ? ""d)	?q!oݤ³™?dÜƐ=?ï¨n£É?€ãRš^"ü?U+'Ö,Ê?[Šø1KœÍ?ƒAVY¤qD?}¿ï"Èæé?ï2)õ`®…?‰vùoÿ(?`܎8¢ì?VXW"?—·EÉZHî?‰(
D®Y?ïfŠÃ4j?o†yg†2E?Vlh¤}O??öáyâG?'ÇáK±?nhß÷7?ï¦ß^Ry?ûÊ;M?:M¶OÅ
@?1B¦WgüÜ?…¨ÚlW?Ïΰ¹Þ?ï¯&§<M?•ñóGÁÒÌ?a'ú[|X»?k«u
š¹?š¹»æ2=?"{Z	"øÚ?î‰ya¦õ3?•=†þtU6?dDj±°Vì?cþ'"§?¦$#=û@Ü?"úIqÉ?î†W´™È?Žܳóؗ?]Ü­B«dµ?X±é©h}?¦«©*u
b?ÆM'4CŸAGN4FGL J0500.9-6945e¿ÅšH~|RÀAeÕQ֌À8¨7æ÷~À;v8è†@~ÕØd/ª@Óo1?¦+±^²<ÿ?REbåÇRa?³WÔþ©c@=`4H1?ïçë ÊÐÉ¿Þ[]‰H¾¿ã»üР–ä¿àô÷Ãñ[ø¿áF]v'Ï¿àïኟUNASNone3FGL J0456.2-6924LMC-FarWest?í2¦"e
‡?­'ú_€cÖ?cEêÄ|?Å?W扝1X"?µÐœ:¿Š?­>­­ÖE$?ï­þé)¤¿?ƒ˜x[UA?U«¯
ѧ6?b·'˜fpO?ÊÏÞÛ[F?€g¬áÐ?ê춢?°S†¹èЁ?Öü,Š^?‹ëRmüK?ÅîÝcÊ?¯¿}ª‹ël?íëeS8X®?¾çÐÌ?~$­¾ÿ˜?`ù–å£H?­…>ã?ŒeêÅ¥?鑛þp*W?»º¯º~|Ä?'³òú §û?xKH9gó4?ȎP×=$?»
E°k÷?ï_J®F?œ…œä]Õ?eŒ«h%?t¾8Hg–?›â‰1'"?šaKW¯D?å"µ6®÷?·ÆÙ÷A?•5Е…î?°ù˜Ãí?Ôj'5¶"?·jÍç?ëÍ<Uh4?££hÒÙ¤?9Ž8‰Ö¥?wnJö Â?½‰"2H¹?¢eNMëÆ7AGN4FGL J0502.2+3016¿ærý7½uÀ+
€òçÀ;)ÿ­Ê©À<7b• Ž@ Æì)Œì?ùِʽþÔ?Ù¢‰bñO?Úìåq?ûmªx.—@,XÛäAÞ?ïÿùëñ¿ïýÅB"Ð?ï}[À›<¿Öèf»ö»´¿Ô©n)©¿ïý'€›pßUNASNone?æyXª;?Æ;¬"éðZ?qeeƒáx?nÊÐX?ÒÈ9¶kG³?Æ$¡üOØl?å‡øUwçÔ?Æ®‡õ#Ða?|ž7¹VÚ¢?ˆ· x'‰?Ô}–vØ<?Æ(˗(â3?êËÒ8>e?ªGÕT aÌ?‹ÝŒžÅŽ¦?…‹‰'ßב?ÃÞV.'A?©½pò'?ë¬'QíLc?¡ÿ闤E?`"ó0;?P†'~Õ?Á
"'¨ñ?¡ó˜$ºÏ"?Û<ë¼.Í{?ÈâF5!?~îð(©<?{@S~kŽ™?â#¬BÊ?È»^æ?e?ܗŸSJˆ?ÇýP`ž.?}­z%U?w$ß;N?áz`V,™?Ç¥'™éÍ?åC1ñDR?³/{åˆîA?"¾Ó–¾¾"?‹e†ÌË:Ë?Ô-®ãÇ~ô?²ÅY{qô?æÒWnâòå?¶!`Xøm?cÝTIýQ?aƒ¨4÷·g?Ò5!h
8*?¶ê.…ÅMIXED4FGL J0503.8-7508¿Ôò8ržiHÀ@ztBÇû­À;U­…ߨrÀ<¤¬Okx@ÆWÄb&@z…ص?ԏ&#*Q?Ï1¾{{?ñ'ºÄŒŒk@_[]ˆ¿ïù "_Ì?ïúŒž3‡A¿ãb°Ï@E¿å¡"ßþع¿å"PŸTÄ}¿ÚEÙ]ÔÇmUNASNone?*?qÓŠÔk½?L*±iì?<'yÁ?{)êÁÂ?q?öŠ0>?ïˆÒ"»Û}?…q¨Öü»"?a"°s8|?eçÿAäÝØ?‰jp³²¤¡?'§ªà,?ï&l^ß½?‰‹TÅD¼I?w<]ZLrb?uûF^;{'?•c\ÐùGÎ?…516Å9?ï&Ø1tP?qc ;TÚ?pùiµf®Õ?S=‰oÍ9Ñ?–æŸZ'X?o‰w=•?ï†~&ÿü®?}I·¼î
?[ŸÄŽ_]Ä?M3³1œ?Šì}«Í.å?{²ªO"'?î†á`4?¤°ŠÅíê½?u¼çê:?ƒ5>Nó?¤ÚlZù?¢¨õñÍüç?î™Yb>[?'§9'ÝgÄ?ƒØñÃs?÷Rý;÷?¡ytn¾ƒò?Ð…&
¤Ë?íÜí8'9?ŒStNäó?}£*þ'?l¿¬1-•×?®ŠŽ©oˆK?‹[ÂZ[€AGN4FGL J0506.3-0620c?âWŸ¨k2mÀ:6ŠçO/À:¦IÚ>¥WÀ<O%üéË
@©{%2h@š±ý=­à?ËnŸšåt?¸d ,?éžu "se@JÖßuEý¿åEv+ÖG ¿æ0©€—j¿âhx>Õþ¥¿æTÑ]Ö¿ë®IW¿ïûÍÖ¸UNASNone ?ïC2±Fù(? ZÙ}$?`[Äÿ¨\?R¤?ùÄB?•Ž17ƒÅŠ?Œhý}@]î?ï§ÐÌê1•?€OÂýt›?XhO§4!?_5Y§ñ?'þÂÛÖ??{¬$3â?ï¿Ü¬òE?‹ÖÎÎL?v#iu¿;Á?v™ƒxI+?–¿*"t…?‡ü°m°,?ï#§ù?Ú?rË[ª–7?má¨ú|1Ñ?ON¹*ýïë?—Î˯µG?qDçSÿ"?íÀX᩹Þ?¤š¤Ã"©¼?uÿ¾ŠÁnÞ?jdœÓ~?°=NL!?¤âK™Ô?îëJ咧ž?šWô›Ž_€?nãÑÿ%…?xýÃ/Ú)'?žº)% –?—žˆ|÷ޅ?îX.
2§?•mõ¸}?ƒb
"ŸÛ+?˜äj³µ?¥¤›ùlÔD?'õ;òB©Ó?íä:_ªé?#؃Ø;?}ý1˜ AB?iS]¥ð‡?­ü³Õ'Õ?ŒÛi‡RüAGN4FGL J0506.6-4629?â6¿Ú¡ÀB{<`ŸÀ;v?""ÆÀ<Ó§<ð@!>÷þSØo?ù(¢› ÚÖ?ÒQ>a¸«?ËkÄIE™<?þ5ctCž»@-œsÇ-¿îm"wú¡?蔩ÀXJD?ïHã—­¿Ý ~Dÿcx¿ÐYGŸœ¾¿ç"…U>÷UNASNone?ïÚțî;:?ko–¢VŸ$?BëBe¼öñ?f DfÕÙ?p>IÀ'Û?^q¾?µ‡j?ïђ¯D¦£?tñ<"k?AcYgúÁ?LÆʎæ?u
FQ1n¸?r‹õç*Jœ?ïXǍè?~+€Jñ ?`¸àHäý?ZüTKrt?'Ð!Ò§q?}0p
$å?ï€È+Ê«'?oñ¤"nŽ"?Fܦø"ì?9aŽ»ô%??Ž`*¨™=‰?oÅ×¹²?ïªË	¼?tBeÃ7ԁ?U0Â@²ó?F¨Æ.ŒS5?'­­H0œ?s{Ú2ï?ïq	cŒ?'ø!$Âöî?SÒ©*ê8?d`÷Vƒ-h?¡²"?ê|Ì^†×?îËf«Z·1?öŽ´Öd?fGQã‹B?dE%KX‹å?¡å ,zšA?6V¸¥KÊ?îòËꤤ?‰jˆ³8Q?L+ŒŒþÐè?J=íy±ùÀ? fE"ý¯?‰ ¯?K®ûAGN4FGL J0506.6+4545¿£5çŸ_L@

Ý8TÛÀ;@{¶YÃÁÀ<r%ÿn	É@"‰ioZUâ?ûŽnD—à?Ö§;®+÷Ö?Õ¥±ÀVò«?òésçXiN@ïÑ—Êâ¿ïÐaò¹F?íÈúz…\¿ð?ïÿþBe«+¿Ó`dYEìs¿ïþpéw'UNASNone?éÁ>?ºà?w҆­&;ð?‡‹ÑB¹?È<skæ
¿?¸AûM?ê ^-̅Ä?ĪÄ9Ua0?{†u "À5?ÖrË¡?Ä¢SžÚîp?ÃÏwêû¿‡?됳/S?§•{ƒ­>Õ?‡`¸Vúâ?ƒÈeãH_?ÀG1wœCÃ?¦±šH?ô9o°?'³u︍?tØèákÅj?o
—"%Ê?¡ÛœËð\?Ün–»·´?ç¦HçØõX?ÃöÉ
"™?Š¤
¡õå?•*ö`µp'?ϼ›ÀÿþÂ?ÃÚ=ýÖHæ?ä¤ê
Œ?Ï «Ç®?"99a¿pj?±LP¾?ՄH<bd'?ÍbÃ	»¦Æ?è"¾'\T.?°pî_W}?"‡/÷Ü?‡LŠCі)?Íp¶|åj?°"é—ÿRÀ?ëù€Uê‡?±=±¡}]?—A'»Ñiú?3xj"_?ºc³aIy¤?®žr…ÿ?AGN4FGL J0512.3+3329¿ëÚaÔõÿæÀLF__áèÀ:v9´V´BÀ;üz,€@ ŠŸb0?ú–=Ć­.?Ó¥àú¬.?ÜÖÈäŠÙ@æÎãþAº@0@0Fĵ¿áÒ)˜¾&¿ð?ð¿Þ¨'¤W¸¤¿å>8ŸÙ¤¢¿ïúúý·¦JUNASNone?âGь
v?ÎL@ufž?~ÔûÛ!1?€jÁ?Û\ ¦ð?Î><*©?æë·sŸ4?Äem¤ë~¶?x¿¤^YS?€c§ƒ2î?Óq±'MŽÃ?Ä*+Ø ?èíJñ•Ú?°K€¼:ôÂ?¦FèØØ/?™èÊÂ!Z?ÊjžœÔ?®]ÑÎ[›œ?ém9ÎÐ)›?¨êo¸Bÿ?zܧ2£ß?i7@ìbù?Ét3Š\]?¨ÞâaÕ;?ßÉ?ÖÛ?Ê2üæ‰Ñ?µ/i?H?‰(=&u6m?àƵuÖ?Êa7Eš¨?ÛD&^þ,?ÉóÓ]ô?€	Æ^æÂ?Œå2!±?âŸ'ñƒ?ÈÙOQ¡Þ7?âñLŽ4G?´4tHH»}?²BŠ‹÷Ž?¢xBVÈ«Ù?Ս,ßî"ï?³R¹×VÝj?ä8k׏É?·ªQó?~&Zݔ?x aJ ù2?×ëÉV™?·Ç»Æv8ÅMIXED4FGL J0512.5-2201¿ìíüÕ¤À?êÈ`V'À;&k&¿‡jÀ<~ž43
@‡k;p|@R ÿT–?Àv_'Çp¿¾,8Ã
@³"ý*bª?ú–ÆXêR?ï÷%  ¿åø'Už˜¿ëÝLâ0â ¿ÞµíãðQ¿ìn<ô}ÿ?é¢ áÌäUNASNone?î¦Ã(7?±+q$W?gM6.…7"?s6q'¶,?¤üjUP˜?°Òeޙ7{?ï¿ÚIž?žL'2ʊ?}òöÉ÷¸?‰ÑUtÈ?•`lƒ?–› Î'|?íÚ	¼q1?žíFŸ3§ñ?ƒ"õçî|?"G¨èAtv?­ž¿ÀÁÕ?ôjښ?î~jàãHÿ?Š©úS²st?Â0Y	?iðÄçЋ?¤!.Á÷k?‡ª‰lUÐ?ìîl$ˆþ?·­õL@÷÷?'ï;é†?'$ýÞ»(_?¶H õÜÐ ?¶¼y|‹T?íÞYßfÐ?ºo‹íÎ>?–~Ã?à^³?§ªðêˆ?±ù\_TãØ?³Â|"ü‰r?ìÌÛ®o$?¤ÒÃFf@Ò?Š~U±½pÇ?ˆr½,ˆÙŠ?¶IWÖKhÄ?£É²€º2h?êIú8?¬\Iәּ? \ææ̀±?'£;\a$¿?ÃË¡Ëä'Ý?©v¸RL1AGN4FGL J0524.7-8304?ï3Ál÷À=~¢‹°£À:Mó™À0À<Tˆ'@>Ãز^7@ˆ$&Oö?ÍÛ·`Ô×?Óù|ƒ3Pº@ÿÞr¿?ü÷f³›x¿àHksì`ç?íÁú@£^>¿àJÞ˜–¿ë;›í0ðc¿ÚED"ٖ¿ï÷3rôcUNASNone?î¤rÇY³?™Þ&jââ?r)­ÛÀdš?l:]%¢_?£sÏ'Öµ?—ùpçDØ?îhà}~o?¥´Ð©;¨?'!tJÓÙt?™¢Õ`!Ü? a=ýNU?˜2|í‰?ë¸ÔÏÇöF?¦>äU´? 'ŖÎ?'±¬¾(?º)Ðë·Àî?£O¯o¹w?ëìƒÐžW]?"†fE‹"Ô?¢ù¾‹U.?ˆlI ÒªÕ?·4†Ç?Ž;ízÈV?ìÊäβfU?¬B0póù†?'£U6©?ŒÑž€¤¤;?µd0µ<ª?¨¢¿¢V?ë.üm?»ö#ó¥(Ä?¬Œ¤èk×?±½—ÎU?¹™
kܱ?°¯©¿@B?èÜr,ÿMº?­i!ACAH?¬fÇĬ?›pe:­«?'nݙ£ª•?©ç©mª?ç'Á	A"—?§y3žm1ê?±Ê²[Öl=? ^Ž¿ùL?Ê{¢­ê^ƒ?¤~™›$½AGN4FGL J0527.1+1152¿é¶s'i—À)[	¦qï1À9Ó@ŽeˆñÀ;¡¹ìxk@Ì´äxºý@‹®9cÎÜ?ÇV†
JÁ?ÈB¡û'Ýé@-©¼&Œ\@*ø==ù¿ÏZ¡¡¥×•¿ç¨^žEû¸¿çâJãS!¿ék8'ŽºC¿ì.4@ylÓ¿ïÿPþU0UNASNone?î%ŸUŠü?£ßGHŸô*?‹SM·pS?vLþ°|ŽŒ?©C5Ñ÷m°?¢'ôû4×2?îðýš2Ø?ŸÕ*^O ?P{UÔM?…¦›³ðÊè?™Vµæ£¯ê?šº¹ò¤
?ëËއ'ä?¥P®[Ñ?›ºfÁ+ò?2"Æ®Í?º¸Ïƒ¥*`?¢¡ËþVîµ?ë†&R¥?—äá9?"È©u±gT?p•qÖ®æ?¾Ý4l î?•¨´íò‡(?ë9p
÷LJ?·œíªˆ—M?'yy5†Q?‡<Ë@
iÔ?Àë­Þ?¶yëÃéì?ìò·DFÎ=?¶·W¡zÚ?›ÁzÂ?¤9֙?±zö'?²	SeSW?æé!ÌOñ§?²‡KI½Â?®cðûŒE!?hd ¬Ó?ÌÂ|¦.[?±>Ëß}Xº?åotŠŸ?ªÖ΋]µ?¦,TbQµ?ˆõßا¨N?Ò–Š×›?©ÃìÓxC¦AGN4FGL J0527.4+6647?à
ý!ÜÒ1@1=¼#1]À:ÄÑ2À<¡S¢>"@›_-b
ç@ŸÅoá9?Ãaó$¥PÝ?¯fÿ0ø?ì(›?6 Î?ù÷Xÿ ‰£?ãÞDno¿à_0?ÿä	äO QD¿ßÆæ#5U¿ß¹"@"DÆ¿éÇaS/UNASNone3FGL J0527.3+6647?îÌ¿O'?Ä5hŠ¶…k?Z"røÆQë?ÝÌËáo?¢b÷w‰?Ä
t"Íƃ?îòÏaÁTã??ÅÂáIX?w¼"0uñx?uíT¾0šW?›¶ò²ôæE?›2ªý82?ïp@U
V2?xåL5Ã ?h8²wV»³?gžUÚK6?á¾e(|?t­Y¸U¸î?îu8€œiû?}ôñåþ$?‹Ìôc4oÙ?f̨—:Ó?¡¹:Û´v^?|¥½8Ýí?îû/¸²í?¹â!sJÙ?cÞs]XÂW?dI4¤éÙ?ž#ë™Jý?¹â".V»µ?íEÛ¨¡Ž?°£µç@$?0º†Cés?"Ç£Õù€?²+iO*ß?­Æ2ãXߨ?îÝ=¼?ˆó¾Çaô?saŽ33±ý?lÒ[Ýlq?T]
»þ?…–6du]k?ë'ûÈ/Q?•ÇZb›,v?¢Š}N¸´b?†"_!'ïz?º*9yô7Ë?–Ä7
C›œAGN4FGL J0529.1-2449c¿Èøч
•À<b›Zcù¥À:µ¡qÕ/rÀ<>ç;
H@‡0Á¾Ñ·@2ÙÏÏ?ńΆý‹¿£<§%Hcò?ÜjyMÉ·@Tgm˜Š?Ù©,߇¨¿çÑxÞc"9¿çÎ0_C\v¿ë]H~u|¿à@".þñ¿ïöÅ>cUNASNone$?ïëUbvÜo?YØ?;¾é?:G	C3ËF?0µª§8x?aa¼%ê.4?X#¯I¾–Ò?ï´æÿ¨í?€ £Æ
«è?RÞðÌíj7?]%þâᛘ?€jañØ7?|Ž•.¥ÚÆ?ïK¦à1·?‡
™ÍoTº?ac8œÇ&?Už;Šß³U?"^¼í¿]9?†‰8«öœ?ïÂ
5óí?Z2}6Ô¬?C²žïjI?-¿ì2"Õd?|ƒõ>Î?XÎ\ÊÏ{?ïÖXhï$2?qn3"§È?JۍKëh?G`­-… ?qxYè¥"?pÂêzL—?ï	coLOJ?¨i`TŸ+¹?bçh¤m(ì?sœ5%×#?œv¥°™?§Ñ¬óx-?îW®I¡V?™Nœ,–?rSåö™?iØo†`Wà?¨D메‹?˜6ŒÃ˜&Å?ï9Jæ‹Ã?{""t¥p?^ëË jz½?QãTúád?–ðùïôì?yÙ¡±îAGN4FGL J0529.9-0224¿ÌiºÊFÀ32 D®…ºÀ:}å‰\4´À;Än@O{h@öE)B@>ñ³/m@ӝ_÷·?êt™=SH@²ß­*p@ÕD¬à¿ÑGËÂᑿÆ|ÊÌ¿êw½ü¥X¿ïW}_§/"?Ñ|#ý`='¿ÆNxÉjl°UNASNone?ë(b"YIÙ?Ã%{W½2?œçjê°å?¶B<û"ÿ?¿ƒß(øz?À/²•iW?îýp0iª>?¯ñ@šZüÔ?"ìëË÷'?—2¸0ò?•Û"öaA?ª÷iŽ"?꜖þ×}?©¸™®Ð(?«.÷2}µö?ž,$ÀšÔ?½ƒÌl™u ?¤¥¥P
ï?î\¯!&|?¤¥£X®Cª?=ðVÅë3?S™Ïå}:?ªT_ˆ
Ç?¤ÛùÉ+Ä?ê&ªí1¥?Ãä=ƒævd?§!eñŁ^?¸=ó{nRœ?ÁÓØG̕?ÀoLŠ"?í/c
cJ?Á'Û¿ÙÊ6?¤™Ñžñš?¹xýWY-C?¨oõúK=Ê?²‹3"î]?èŠê/±|?®þ‰{qîã?´ù˜ù.×?¢õCÚŠÚ?ÃÇXþ¨ä?¨
Z˜?ê…X%tÈn?È£< JV?i8CE?œ¯<ë{‹?Ņ¿»…þ?È)5Ž¶AGN4FGL J0530.0-6900e¿ï¶'ý6·À@:r2LƒfÀ7Öl9äþÀ;;¹ÿk@âQ—ø.Ð@ç±|å-í?¡š'_`D?•¦çÿ¶¸?öÛïqµ@±µ›ã÷?ìOu¹Nk¿Ô\Édb€(¿âµ†à‹P¿á×ÊÆbP¿á"€ãÀ.¿åpà<4dUNASNone3FGL J0524.5-6937LMC-30DorWest?çB&4êdÛ?ÃR:ïY"?"u¢ї?"|ɯTú€?ÐØ"Üü£?ۏ×u?ëær"	K?Á'X^÷î?¬;˜­A‰?³;ζ¢ä?²Êf¡6Ö]?µ·¸Ü–±?à³H&çÿ?µ=µ£Rv?¨c6ŸéÒ?œòEa}?ۍà¨?µ"ê=oì?ä]aF¹DQ?®Æ3¡íü?°-}È1ü_?'»6ÔÀ?Ó9Þ.¦?«ÀƒRÛD4?äpnzå'?Â÷ÒèxX?"˜v²M•?†i{Â䮥?ÕæIƒŠA@?Á«î<Öl€?èS1,»d?ÉAèÒ*Éq?¶QQŒÁ?¿ÑaîÜQ?ʒŠÜ'h?Áیá­ã?Û²ŒI¥?µG×Ó¥©Ô?¤"½­F¶?˜€³xû¯Ý?á0ÊìÅ2?µT³W´?ÛvIR¯Oc?¶iċ¿ú?»Ê!iåªr?¢¾ST"A?ݗ.R×F?µADö''gMIXED4FGL J0531.5-7823?Õw¬5ÓwÀ>…'¢xæÀ:½ÚgüÀ<J=k›Y@ÿW±Më@QÁ"³¦‹?À1{¸ˆD¿°z_þ©z?ðÀÔÜeÇ@õpKAœØ¿Á© ã9öœ¿åø þ¿ê'%ëbd¿ã Å®¿åAÝ¥¸?ŠñTŸC
UNASNone?ïà >íY=?i¨¹;Ý;.?BˑgóH7?8'jo‡6?k,܆¹?h|?CÊI?ï´3¬]t-?~ýÔì;â?Ry8±e}ß?Yj#ëÝ«7?€£íÛe@÷?{G$
œ½?ïXÒ¡øã¬?…`Š{»Ú"?eeÈå?h,cMfÁÿ?'CØ(ðW?ƒè²Æc>¥?ïÆ×â}>?YdÞWå?D÷@Cn¨²?.IàNˆm?yõ&׈ÿ?Wy׫yË0?ï³½/Üù?~*ŠÖOÝÚ?UÇ/Z‡Ê2?Nx­JҊ•?€†j¾þŸ?| âQ…
?ï=óÖ{ø?œ£Ö«†?afÞAýn?pcžÅnA?šKe·nC?›>Ñ"Ò$ì?î°D½"õ?"'¯
]ë²?tÔ²&ÚÜ?uۗ›]®"?¢aë"Ú?'fQY5 ?ï3yÿöDë?}w†ø>Ùò?dW'¾,@¾?UQ½8
'˜?—ÍÆÞ%"?{Žn_Ã	AGN4FGL J0531.7+1241c¿êè:Hr¬èÀ&Ž·ˆ—é–À9Æ2Ôh£À;iÏûUvT@Š¿šàª@·V¾È'?ÐxR!5î?Öܒ½‡_…@ìÝÿ$7î?óᣖr¬?ǯ.–ÁM¿èrd×-©¿å—˜Ø©yá¿ë{Â)°¨¿ïû¤üۈ?éÛG¹ÒõUNASNone ?Ú!t¼6ôÖ?ÌIvZiç?©àÙa?;þ?ÁE¤­|ƒ?áQ8µõ?ÌåµLû—?繎›í:?ÉßòïKQã?²°X•ˆáè?µF…&Ü<ö?ÇÕz"àf?Ť$¦Â;?ãÔX†B¾…?²(ùE?«ç–»(?˜Oï+œeý?Ô÷ÿÜĒ?±¹U€Šàá?وä½.t?±hõƒ°?·¿Ýéå?˜žOV›?àD1hz4?²˜ñë¯^?ËKX£°ê?ÂòÐÚ	¹?´…ý1N?­€yNTߜ?èE36…›?Ä
Î	bÕ7?ÞÜÞ«\e?Ño
æÍ?Çö'¡oý?Ç׀|^—²?Õ'Øâë?Îbò#ڌ?ÚU‡ p7ö?´p4}R€?²AÀÍa³~?œÔ6Žâz?àV7*u?µSÀ"?Ä©vË'J?©J=ɾ?¼‹Îpw?¥œd®Í«?ç{Ä0"h?±õ ·§>MIXED4FGL J0531.8-6639e?ï?Ìw1÷À@K´¢3œÀ8ƒE§©ý•À;ŽÊw‡öÚ@ÚùªPv?ÿɌ;E‰?¡þ¾›B!?"‹|ÂÀ¦Æ?äˆô'
´@‡ÒFß8?¾
è¿×È¥`LEÿ¿áG
À²ã¿à+7GMœ¿â†òÍèU¿¿×Ôþ_
UNASNone3FGL J0525.2-6614LMC-North?í"ðŸå¹?¤QñÎƙ?b…3è4?U	(‹Ði?²ÄQaÉ(?£ý~ãîy?îñ®xÎ?£êÏ%Ég?ŽM¿µ9ï?ƒùÄÕò?™ãV΄7?œ-W´ÄY?ç+IÌ@¤¥?³wçú?šýÜ_1?•6›ÇFä?ÏóC‡¿'?²Y?Ч,<?ì'îõk§n?—åÈ8–Þú?šR¹á#?íÅñ1u4?´ÓÚtVJ?"ŠÉB	×ô?놊½ÖT?²…öM\{Â?~Îlä̟3?rÆ¥aÀ¹?Àïa¢1m¶?±í¥ê?í+yÓ"Ù?¸Ÿ;¬èH?"Ë—ÁÈÏÍ?¦¦‡ܜƒ?±±KtWÄ?²±¨qÔ#?ãÂ(:þûë?·f›(«i?•ê.aø?FŸ¾ÐŒ?×§û~ˆ?¶ù*Ùrw—?éyL¿²n?ªè.bul?ªï,Uðä?"3A~ƒ\?Ú¾ÿüòQ?¦YßÀ%'¸AGN4FGL J0532.6+3358¿¹:;éyÒ?ÖâЯ°\TÀ9Õ¦k93þÀ;e·ÂyŒ´@Fj(ìç@'¼!ƒÞF?Îá\PãÈ?ÅФ®§?ö$SN[®?üÔ!s€¿à…°¾¤@¿æEMFÚ¯ä¿éùŒ|z¥¿ì}@"Ó¿ïÆa®pÁ3¿ïÿWƒuUNASNone?è1Âñ
?¾ÖZ»É€x?˜Ã0,GЇ?›´pL¨¬?Ì#BîDÊ=?½Œ<Â[¸@?åÆGõ.)?Ì15—'?"5dK˜«?"ÌÆ>Ï?Ó@¯µ…?Ë?Wñ!?å†ëÚ.4F?°\—¾×?©#^A
mO?˜JÂc?Ôý?ÑͼƒJð?®xΣµ?è§ÞHu9¾?§Ug]Ù»M? ¯Ø¿,!Ý?€Ï¦‡òà?É4¯©ë?¦rZ`TƯ?ã叿ƒÁŸ?ŝºVŽ¾0?¦«#w?¤Ã*=ÿ?Õs‹x'?ÅL4ÃÎmÙ?ÙVIŸ9?ÎÝ0˜àGd?£áÂÚ}?®µÝSN?â68Ÿ|?ÎçpǾE ?ݲÏÀÈ¿?²ƒ÷ŽõÚ@?¶'çwÂs?¢gº¡Â?ܨ¶a?Nä?²GèÜÁÅ.?áŒ!˜Îdõ?µ˵&'/?®Wõñõ?–bUŽŸA?Ù¾.EÚø?µ=j¸"VuMIXED4FGL J0533.6+5945?¼! Oðr@,UîþOü˜À:‹øÇ&›À<Y>Y#@"yq…ÿ3@I©¿Š¯?ÁczcHyÁ?äF]²b¾@©†b…0V@ÐÎí
Š¿æSø`îW?ʊˆD1³+¿àKý"z¤¿ëÑ q$0¿ïÿ®2D¡?Ô¶0=µm5UNASNone3FGL J0533.2+5944?¼xã¹zµ?¹9"Ës>?ëE;j܏?À-'X­k?¦¹æ"¾¨?¦§Bc+?¹q+‰*<"?»%Ô¿¤4?éÍÞôÜO;?Á¹T›?¸ÜÐÏ0—?³ñÈúm4…?϶A߸%»?²T9.Þ?äžH*™º.?´¢uȲuƒ?»¡:ëÁã?£7{Çjšû?Øiæ©þÒÀ?¯8•ý²;?ßÑŒ‡Ò?¯ªÊÜ3?¿ÿ*0ïÑ?šL'TÖÆ÷?©åÎ0j¥?§î' ¹æš?ìh±H¦¦·?¸áV&NÌ?¯Õ¥­[ë?®ý€òÛ_?¦'昸¹"?°m–©3ÇV?ë±­ýÌ?À*?nªØ†?·c/D')‰?¸A»—ËW:?¼·¶G¿Æ?§rs{QùÖ?èƒcaE·'?±ÀږE'?¿-.®¶ƒ­?§¤UnÎ=0?ÀO[t'EŠ?¢lÀ«Rêä?æ]ì²pU(?±›%?ñ?Æ8ñ¿†¤[?¨Žœ-͸PSR4FGL J0533.9+2838¿ïz)âҞÀ¤ì¦†çæÀ9@¹çíºƒÀ;!ÂÀ®@ƒvÐ@	ðÉS›‰?Æ*<Ó¿(ÆÚVM?Æè6 %#ü?ñ9"õjÑ¿á4PŸTÄ}¿åi¤ßGú¿ê#OÆðé¿ïúk _pÿ?í®/ªè¿ïÿ«±ÊUNASNone?è\|0…·?ÊéNÃ\‹œ?³8I¨­˜0?Å}ôÜz-²?Äóu:6?É7²ä?èà‡Ge!ö?Çã&ëÒ Ÿ?zmܳ¾îœ?Œ¹çêJç#?˪sü§?Ç{å]?â/À8%ª?±ô8f¯Ô?²'Äîš?¢<ƒä²Žá?ÖûÎpC'…?°ü¼ 8?îaËq·?¢G/lé³?FØEkˍì?G峛Ӯd?¥ÎœTAÈ?i¯ÁÛx?ç9ñؗRº?Èræx*Å7?°ˆÌ¾ÞBX?»"$EW/?ÊÓÒ>j¬?Äñ•rÝ1
?âm$¿À¸?Ðsò-âï×?‰õmkB&?§Î_ªµ_?ÚV€íH?Ð…Õ¹ÒÁ?ÜՅ
ª?±áØóŶ¸?ÁqSXûš?«FÞåíÉá?ÚqÑ?3'Ë?±Ï×Ñà?ë›p˜æ¸©?ºÔbWãì¤?lЮ=öqÀ?wÊ]mV¸?Áúâ3ç8?º­LÐàAGN4FGL J0534.0+3746c¿xq\·Ü"@4òd/UÀ9£¶"|#gÀ;c¬sßÌ@þ©éèß@ϒ¯šŒß?Í7ÿuÁx0?¿Þ-G#*?õ{¡çEô×@	©f®ƒa¿à˜›ò9¿çò³ç#¿çCKK¶¿çùš‹1!
¿ïûdŸç¼g¿î<Ö 
L	UNASNone(?ïÀC±§ú¨?rƒ@áÏlÕ?@•¶?8ƒ
$‹A?}˃ۜl?qé•^7J?íòÁ•%‹?°Úd¢wB?f6V›pó?rŸGÉ7Tø?¯pAdøs?°>dö–ù?íՕº«¦Ñ?œ?þ¼–ÆA?€å'زY?~Ã2ªT?®mCÓ©Ó?šU#Ú
?îvðÀO™y?ˆ¶È·;Œ?kç%ÞÌל?L¡9M×$?¦Ò›	Öú?ˆ	iv–SL?îÁP‹? è®ˆ5?T"+rxY4?UøBtJ°?£IíÄ? |$äq÷B?êXђÚ7Ä?ÄwIÙÏ?'Ð×{c?–ÍÁƒ1g?Å{\¦¸Õ¹?Ã=k_8cŽ?눊Ûç?©ElÜ!S?'éNÁ6Ê?ŠüœÖâf?¿:¬õÓœ?§\šdJ?ìtõ-q°Ð?¡¬<íóÃD?{Õè—À
ê?gHÝè5?ºšø
à{"?¡N[³AGN4FGL J0534.2+2751¿ëÐ/@ÆèÀyž×ÆûÒÀ:e:V=#wÀ;ÚØä2D @"&H?"?þ
Ÿu{­ ?Äã׫M D?ŽyÁô?ʧÓC3†j@0a"šK?Ö©Ù‰s²¿ì+º~¯•?Åû…‡hêz¿â©4wž¿è
ŋë›?Ö¸qËõ6xUNASNone?èP˜²¤)?™ÞkŽL?g
£ÓÅ?X5Šõh¬¥?Îa5È	Í?Âœ¼Jë?ߵ݋Н?ÌPƒ%8ô"?€ >³?‡)ܺ"	Š?à0¤‰ÊÖ?Ëú½<‹÷?êÌ_-P½?¨K•ëVZ?‡#""±Õû?.6R,1´?Ã\Jl€i?§v§¬JÙë?è#å=îm?¤ÑüK:r	?€bÅâÂÁR?iSö<å?Îj>©O˜?¤Êr·O–?âp­´{?Ɨ¦Ò^©{?yœÔa–ç?pS|˜ó§?Ûz«S¯a?Æ«¼.Í{|?ÒI"åf?ÆÙª"JO?w{Q‰"f§?…õ~ùƒ"Ç?æ¬>êBöÂ?ÅþUV¯ËE?äùË˚óŒ?³XºèZ;?"6ø2ØÏ¢?‡]îÊWå`?ÔÈøå¸Î?²èÆ¸ë×?Ýàð:Ç?²/P™ñ9[?ŒüÓNò%?'bvÐÀo?à›"•›)´?²…‡NIWMIXED4FGL J0535.1-5422¿Í"ÿU$
•À@XÍJ¡À:V¶~¡ÇÀ<LtÎ6/@ÁV-ßi@qËa'Â?È;v8@Ž;?͈Šèü®<@]GóÐG?þvyÇQ¿åèÅP׉¿èaÊsc¿ãèS;wG¿ä«Àb±%¿ïÿŸóOîU¿ðUNASNone?ró+u? KüNaæ9?…#¼?yt"‹ô?¡LO©Y­?žShDÓh?í²¯Wúp}?©x^`µ?›ÀC¼Ky?w>ºu¾:?¦ôè¤ã‡v?œß'h/Üj?íˆÄ½tÑ?â;B"Â?˜k'öc ?b:"Áì´?«4	¿=å`?˜ÛÆ¢¬·?ìKêju?'i
G¬¶?£Tv?'c¬âö?´§û6a?‹<Tâ2ú#?ìVE)ˆm*?®X5Þúšè?=ªhEz
?'2	/?µþl‡,?ªs|LÍP:?éîw!Ó?½¤î6~í?°åa[I.?¯ÐxSÓۘ?À?°Ç*ù?µ·0³´?ëFÿx›*?§´‡åõºB?§dù@' I?˜PgŽ"ß?º‡™Ål?¢±ø50cu?ç47™c,º?¨9õ=[
?µ.:Äeø?=Jßv«?ȘŽZ ]?£âóRõ%AGN4FGL J0535.3+0934?ê3oәçëÀ(@ÛH'ŠÀ:ìÏ¡"cÀ;•HFÀ®±@ÜѪF@¼mFTx'?Óœ"$'?ÝÝÒä>š@ko\¯-€@
kSù&r?Ñ{,܁ö¿ê5†öÿ¦¿Þ¤Cy|n¿ë¯
Ÿ$óÕ¿ïùu!j2ú¿ïüZžÜúlUNASNone?ï½».a4? ©}êËí'?]=j£¸'?aéF'Lÿ{?šÔqö?õ?ŸÍý›ào?ìªhâþ£›?ºg°Ñ1?íq6'ò?"Ó¼iÎú?¶ï
ÂlDÎ?¸jŸCOÿ?çëVéNkQ?¯¶ƒÖ«÷)?©F•¼Áò?œ‹›P?ʶ×ö?¬Ü·Ý+?êÝ?ò?˜ûήSƒî?'Ý$Šƒ9!?qõ?Â/ëPך?—Óö—‹8?íÊ$¨ù*p?¬ÆMS[Kõ?tŸ{Zê1b?síüû¦'?°dãã)?«ˆAyb-?鍣{3–Ê?Æ
Vؐ?£ÎPº*?­ˆöµʘ?ÄÕÞ—Ž?Ã͜jy	?åâˆË7˜À?²é+
†?«®mgÏ>?‡"[¼?ÐÅ ¼Ê1x?±êW1?äcÿɓ?¬°+ƒöËø?¡(å¿l?‹qFÉk?ÕÇC1>M?¬/>lEåAGN4FGL J0536.1-1205¿Öó;ÚTRpÀ6îיåÀ;\ÈWóÀ<†	g‡Î–@ K‹&5è?úV.u^Pî?֘"	\ ?å,Ýُ~@S1B˜+?üšÙ4ºð?ïÿë""i·?B;
ó?­x®ßÉK/¿Õ¬·¶Ì¿äTïE™¿ïþõU9UNASNone?ïI9d+§?'Þہ#4?bg_–°´}?d4E7²ÀÒ?"‹çˆ?'Ĥ赿?탽#â]X?²
ä?È&|?¡{d'!Q?¦–èw=È9?¦HÉAƒ×0?£×¦Â"'?î7³Oo¡E?š–ò±t?†Ûßùˬ?†Q"¼øË?¦ÍÓÿqÈ?—P©ö±?ça;ëNÔ?¤õØT's?¶J2À¾îà?™ïD_Å&T?Ƚa±-þ?¡§Ô€+{²?î"ÆOžè}?¡%üŽ½e?uf¿=tU?xk©@à€Ã?¤Ã1? •'֏jØ?éüNÑMÌ?Áûð•mª?¶ÐVÅv¦¬?»
Só:?¹M8dÚÑñ?³Ú䌍ë±?íƒB/­ö&? b¶®}Vm?Š¼j—?‡ÒXpè?°Ža0‹Qò?¡Çˆ?àÎ5$»?²-þnoI?¼¾/ÕIŒÖ?ªsPØ0?×4e ¡SU?²´Ò¾=ÝAGN4FGL J0537.5+0959?ë–^û|ÒRÀ&î™côÏÀ:#"D¾ÂÀ;œž%"ü@¥¾K°9@1·'¸¬"?ÊLå`íU®?Â*LDQ=µ?õ¸ÜÀ_×@"Äõ=l¿Ð]ó)®¿ÛëA,:¿î]©"â t¿Éíp†OåÆ¿åc¶ž78&¿ïÿöµšUNASNone3FGL J0537.0+0957?î¨|Ïg?ªwAñ`,?ZŽÑH@cX?aƒRVKS?¤«!¦IԀ?©¬~qÌ«R?ï/UxW™?£½·þUþ?Qýìš%8?jM;	OæÆ?˜õ×"Q"?¢Nhã4Â?ëF:Òv?©˜»®'æ?‹±7^Õ½%?‰œŒäs?Á,jÈ˶?¨ÔÿøÓxÔ?ïb.úî?ušï:Ñ^?Vº]«w'­?@š&¢U ?'Nzå¸üÂ?túPwÎ+?î°l_àÌo?§…P렐?b?ÙÒIY?g´#®¾î`?£Õ<d¸¥ô?¦ô¾?¥P?î:càhú¯?³îŽEV
?cUÓõt±?w!­fån-?«$d¶©mú?³Zå¼5dŒ?ꇦõD2?­,$š?ç	?—wlþC?'ETH›?ÅóƧú?«âZn.³|?î"5L?"*ôãPΣ?uG?û/Æ?gIUT`w?«.°#9d?"˜P26LÝAGN4FGL J0538.9+3549c¿ê7è ú@x7~òNgÀ9œ#…}ƒÀ;'<ðKW@\лnÖ@ ‰…O_º?Ê2(œ+o?ÕO´þÏÔ>@é>›A?ÿMðbF?北'·Ôî¿ä‡%"Ï8¿á&caNN˜¿ê^á6çÚ¿ëE¿&ñÜQ¿ïÿm²æUNASNone$?ÆéÕOè?µÏ)‰S_Õ?ʍŸû³j%?ÃxßqÉ?ãÜ]‹ÌQ}?į{á«^Ç?Ôù%î¬?Ç'Gý?ÁÎ)òÔ?¶úcxÀ?áæté‹õ?Ũ‡Rðö?ÒþÍñ![?°—ÕÎlùÂ?À~ÆY–e?¥<§ÞÓJð?â`çqç¹?²yÜgƒùž?Å}ouxb?˜n×®e6?ÑvñŠ,¥?—á&àXj?å¼FfZ–¾? _ÃY'?²Úuòiw:?¦—ãÕà™I?Ç6ûƒˆO?À¯ÝÕÖM?çäc'íkå?Á¨÷£˜©?¼Õ{±u?½Æj«çÇ?ǔ›<Ú«?ÁÄz²'}µ?æ€)Ð!Úµ?ÅIiOу?Á§Šf(†?¤»Î'æ*?ÀÎ
½`{É?¨ŸW<dÑ?çb™÷¿j?°……BM.?¨EU³¢?†Xy¶Ò¼?Æ.Á«ÓÐ?¢ò?ؙ?èôžÿEV2?£Dc˜OTHER4FGL J0539.2-6333¿íÊn= IŒÀ@	d¾ÆyÌÀ;$Æ>=RÀ<Æ<üàÏ@<YC=A@0:û~'?Ë-‰ûìÊï?¬a´Mzª?âùaíÍÎ@zê,>¿ïþøÞ΂?ïØ#½Ÿ]S¿ë=nöWá¿´M"O£¿ä5o¸õs¿ïå`³IUNASNone?ïڝR'?e¼SEõa?4M*Ze‰ï?(øKÑ;öä?ql¡É%éÃ?dífÜE?ïÚNÑ'+?rJ᧽—?:h Xñ1?DÛC%Ð9`?q2
qj>û?pÀ©ÏVõÇ?ïd咖p?€F<j‹"n?c#Ksð·i?c`ݨv³?þä:ìSê?~ç>5@cÓ?ï»ÉҜo?_ô>÷¦°ÿ?W¨~x{ÈÀ?? É*Ð_3?|0÷15ë<?]Aª7c?ï¾ìß籫?s\('ãæ?CÆC€e?<õͺ?~ǜõ	?r~µ|øóÍ?ïn)Íȏ?˜­ÆqÄ?P¢(ÒèµÙ?b3¸Règ?'0£»ûQ?——ÝfSð8?ï
XÇÜ?ˆj¼PA¥¬?i쥚ÿ?h^%¶¢?›@Ô4ëî?†õ;cªà™?ïZCC‡ÐU?yr‰ÐîÖ?k/Øç3•?[Üb©Ò?'W''Tü?w4œ	K†NAGN4FGL J0540.0-7552¿Æ Æ4À>•#¯1±À:J ˆ5ÄÀ<Kìåq	@95:õIn@V—kÁïú?¿ƒ˜%{:?Ì#îX^¼@

òzœ@	N'î['οt—ˆŒî¿×9_\±Ü±¿ä/µš &¿çÂâh?"¿íÿ8$3»ï¿¨'õ:ªúUNASNone3FGL J0539.9-7553?ïdÃÍähº?"â¸)NC_?{¦ƒQ§?qûš
ß?‰K¹?eìO?}°´gÎ?ïx	‡Eâ–?Œ•íù©_ñ?j7¾)JÕ?t}Ñx[C?‹o®ªÈ?†Ð¹]²¢O?ï(«¯¾œ?
£§p?†F.®+[?…"Ñ Š?ŽåTÍ"?…
⍕?ï<É_ŒÏ?lI‰ãÐi?s·ÄÙ.Ì?QãZˆ¯·ù?"xì¥Ûo?h·Â.?îP'Ð/`s?¡)‰€ÿ?–*Žµ
?'ø2ÉYdp?ŸÝ{iÚn‰?•' [²"?î?+;ÕC?¬­Ã?áq?ƒÁ)u‹?"ÏWWÀ?§Òå™?¦®,•¯9?îÞ8sÔ?Ÿ£?Ëø?œÕð}z*ô?–è©ø•?ŸG󹿌š?'(|i먛?íݺ5Î÷}?Šª
0Ah?‰®äJ5?q}h»÷+·?«¸£°šd?†C1
äÑAGN4FGL J0540.2+0655¿ìÞÂÒŠÀ(Ü6q¬À:µ|8_ÂÞÀ<<3Ð$ë@!¼;ž½?ùcㄟ6'?׺àK}?ÍèþNe?úÔg–NÝ@[¹'ï?âˆö~vþd?ëȀB_¿âîà]Mc¿ÕmE	­¿ÈƒëÝ^?{¿äK™[†9UNASNone?ïM菉ñ?'"v	©?UäºUwí?Pz)Tø«Ô?"ã¿Ê´-i?'˜Fã]?É?ïWÖÝ5K?¥¼?č¤s?XfÝÔaä?t/+
¸5ú?"~¶ˆJŽZ?¥"ғ»R4?î_®ž¹i?™e¼'¶ä?mk¼ƒ'ä?rÖ!.ØÁ\?¨.ZOd"¿?˜÷
Pƒý?íùdÌÍ…?Š[<˾E?fœ§ÊðÌ?T³#±Ë?®ÿè´ÞV?ŠxûöMR?î?
~e-#?¥Ø=û*†¦?l¦½Š¸?dùj¼†Y?ªEO>§f©?¥6:–ï?î â©\?´yšÃÈ?iP—^ª}?,öR_!é?¤\Óè
p?³¦|âƒâ0?ìjÓûëp?§Šiá&=Z?|a§ƒàÚ?€ÌÇzo¶0?ºãE¨3mô?¦¨§9ÔÞ?êÁ.R?¤N<Wî˜?r:°ó*ï?l¾Ï\iÐc?Äiraü¨?¤Gwrû–AGN4FGL J0540.6+5540?裗y%RA@)ægrÕàrÀ;u"ÁËèÀ<VòQÁ"´@s"à?@¥vjNR?Î7'^"´'?½¦ù>ì?ðÿfèle"@@o7›LÍ?íc\%šÄ<¿ÕgnÙ÷¿çùƒCì¾Û¿ç¡Ó#þâÊ¿Ý5ý''¿ïÿÿ)@k*UNASNone?ïÒ5—ïþß?mA(ÿׅ?B…1Dv-?4'¹ˆü‹?t"þŸDŒ?kñUf
£ö?îù}±Ç?¤êƒÔ9?k™{¦'g-?sç,(5Öâ?j€Ù,¢8?£È%rBw?ï@GÐp?†Løy?i`>Qôè=?izrN´h‡?"Êþ9®í?".?Dˆ?ïuõ‹Ãÿ?e<çCž?Zfóƒ2¹?A(}´Ñ?ˆÒUÊMEÍ?dòϨºÃ?ï™):û˜V?'\Ù½z7?P»Jù‹bB?F6'u|A?‡žGáè~3?¾ø^Xv?íÍó}抹?µOá°×?|JRnjÌg?X [äÆ?¯—}ӝÿã?³îs¤ö?îT>¯î4?—c÷é^''?z"µ ¦?uèÝkás?§wÇÀQ?•†î´7±p?îP•Í9ã?…d53¾sn?rµ›ÝÇÁ?b
lL§Ëþ?¤¤BòœSÙ?"†à'ñÄAGN4FGL J0540.7+3611c¿ìFz
»£b@}úâ~À:Ç=@Ó/À;dS‹'@'Œ`÷@‰3¿Â?Ðǎß×@™?àtüÌnØü@4zøÄ¢?ù¢îA'šÈ¿ï÷"}~[?ïÏü'$y¿á9NÖ&é¿ì3шô/è¿ïñò¡ų?îÞëuUNASNone0?Öü×_*?ÃÀö)è\?¥2XfÐAí?ŸÞMò‰òH?ã©\¡é?Ã˝iâ>?Ð=!m&ã³?Nj*¶7	,?ÌLcD¦?ÃÍM?àÎn1$Ôå?Èûí+'ÿ?ոɕ_Î?±Ù‹ñ/?½¾®¼k€­?£õV¿
‰Ÿ?ákÅ]¨Ý?³i#2ž³–?ÐïÆPJ´ô?¨&­îÚ!?̈́â4_z†?§Fó@•K ?à&äJÂÆå?­fyž?ÀCF70î?´Q;Ô9?±•¿DæôG?©t>+¹á?é¼v‰°S¬?º$Š›Fd`?¹'«˜>|?»¦ª¹§?ՈëOÞ~j?Ë:OFº#¨?â	4÷OúŒ?ˌñuM´ê?ÄÈߜ!"(?§ÂŒµŽq?ÀO<já ?§qZW±º?æ¹øþÈ·-?²YýS›?´W8 ˜Vó?–"QËßü?Ñý'ïÓ¯a?³¸lehkx?ävOsõ_?´8㯇ÏOTHER4FGL J0543.5-8741?ÙgT®—
À;ÈCރÀ:ÿƒ~`À<h30®ôu@M²³ñ߁?ÿžÔ¼…Vì?Úp™›&?ÁD°E­‰?üg+ˆD@×®7`iw¿ã}ú»×\¿ép|4.ö¿ß5ßJ}Ҕ¿Ø~ÿlÅ¿è9¿¾ëc¿ìA\[ðlUNASNone3FGL J0542.2-8737?ïË͜«r?hM}õÃÍà?S1"±²Cü?NcrÇÌ?u¨´Z‹Iô?e•³õ"?ï­ã8Q³¯?æVŒ¯Ëg?WU"çvŸV?]çŽÛ¬¹ß?œ.M?zÿé÷)h–?ïh¨"h?NQj€zW?eõ—þÛ.?f¼2ñzô@?=¸é³-?z¦Â‹N&ý?ï3,Kk?p\ñ°wz¸?tmæ ýøÔ?SàӑÐ^?"' ÆÃû?l¶÷%L/?ïh
»ùH‰?ƒ›èaÔ_?só°°ô>€?rm_zÌp?Œx§Óæi?}çsŠÇà?îô#ï&¦?›ô-‹iÛ/?m‹N|‹©?vrfӊ]g?ÊRâD?™SE°
	É?î¿õVŒ\M?È¨y&²?{4·ØÀ?|ã~[¤è?? š¶?‹3'Ûpõ?î}eJK?‹Œ'OF"â?†cߥ ô?p;I{¢ÏU?©ï2ú?ˆ9š?+ÅôAGN4FGL J0543.9-0418¿»ÆóL›íÀ0ú;%oüÀ:¬	æ~À;©Jß!c@¼Òo£üÊ@‰4\(?Ì
¾±:u?È·~Fï"@%cµ±þ@à™+µp?ï¿/À·ë"¿Ù­ÜÊ5ï¿éŒÏƒ³~¿ædËÇOh¿ïÿò"²¢?ïÿ9fS0UNASNone?Ãܧû?šw*‡Q¾E?ƒ'Oáß?€?}lrƒ¥ó?  ŸÅž(v?—¨UåT?îõíkd
W?¢˜"z¿»w?…–~å–ÐÅ?ŽV7a¤?–w‹'È?fùÁôíØ?êâ'ZÏÉ?§Õ~«aô?žÎ˜@%?«"°<#?À›ö`o"?¥¹má9Š?ëÁÛ­?œÄ Ó2?˜ AN_ü˜?xŠ"7HOÕ?À×äÎ ^ð?™ÕO
%ß?íß	±'ï?¤!Y®&e?"ÁvÇ @?fƙ¾Ü?§®³á]Ah? c7Åu2?ì—4Å՞?¹þ	r?¥'Ù´WY/?°Ea£§ó ?°|òhï€÷?±i¢<Š²¼?æˆû8'e?²=¢ha¨?¯Üù$J‹?œ/д*B?ΛÞÿe?°àtˆ Ê|?â©pŒZö?°j(/!•L?®Ü˟/˜?"'p[}lL?ÖхsœÚÂ?®®I¼ÒýÀAGN4FGL J0544.4+2238¿ïÇZÄ¿®À3F~i'À:YËUÔGëÀ;ˆöšüp)@ )¡n@Ø
±?ÄóÈd2Y™¿±{PƒP,?ê+Xx`å?þ(V˜½üz¿ëþ¢1ìÞÎ*L…¿âÐÞßôǾ¿äXxœÉÏ¿éÔç¸á]~¿Ð³HAbJùUNASNone3FGL J0544.7+2239?Éæ¢KnéB?Á'—;4MS?rZÐÙ;c
?o*6Ӆ\y?éa¡ËlOŠ?ÁÕj¸ï?âýr™GÅ?Å]^ZAY?ƒ8Œ.?Šbäí]{?ÙkT¡0Ö{?ÄܨÆ÷ån?á³DDAgB?²ð
i'C?™Þ…ìDŠ"?Žü©Ð ÿ?Úûkò?²£#†òìÕ?åَ °þÕ?§ê8sˆ·?"¯™»%Ñ?n‰•æ7Ó?Ó§ièôB)?§á•øŠ4?µÿÎVw¡p?±íVu¦¢?'÷xŒF?صI®¨?ì÷êWw5A?²,üt¦æ?ÓVÜi¼ ô?ÄL8Š,‹œ?ƒ»¯ê!$?¶ãlуy?æ£C'6?Ä;ìӆ?Õ¢7§%C?±êh#ùÜ?£P³ä­ðè?'Æ=/™]?ãùØîð?²U‹N–ê?ÖµësÑ?±•B'Díb?"w‡!Ò¸?‡¯>Œü©ê?äNF‰ý?±ñ›­'èhMIXED4FGL J0544.8+5209c¿í‹hG"d•@''éÌ·ÔÀ:´4osUbÀ< ÇË)_@<Ä~¾Ý@õŠžT~?Ȥ֎—ˆ?¡ä´Âa[\?Ò6§|0R-@9ÌÕh¿á_ç@ìYZ¿â«Ûmi¿æ/Pà˜0¹¿ëù=í¡Y¿ïiОh‹Z?íÚ¤ü¤*íUNASNone(?ï9†«Í› ?'_mO?`50 F0?T§ŠÛ×$ì?–ÌÃÚ¹38?'½CôŸÅE?î…)ôVdÍ?­ËÎ<fø-?~qž0Š¿ë?"CÝåúÌ_?£ß,õÒ5µ?«ŠfsZ?î‰á›™¤?'Ëy?…¶´¡K®n?'>¾ÞìH?¡ô9ðá?€jeÒ×N?ï(jÛý'š?{ᄞn˜J?gèjÃ?QS'_Ñ¿U?˜ç€y¯f?yëØú
Ê?ìÈÑà)mY?°ÄC½?u•"d~/?o¨mC¨£?¸` åÉ`?°nAi©RN?ìMe™Àc?À|ïÝъ?"Iê{?žHúŒüçÂ?¹¢Rêwqj?¾í9ᚆ¡?쵚4ãÑ:?¡€®Æ ?–b—ú³?Œ€Ï
Xã?´Í•±˜îî?žHg–ÊÙÄ?í(Õ¾&Û{?œYx¨n…?,í=?"…?r}\OHÖö?´"´fQš?›¯déªAGN4FGL J0545.7+6016¿Ç;ÝÜi¢Ü@/yb(D€À9Êãv\}¯À<P•V=ú7@Hñk<¹ð?ýHÅ¡_`¹?µ–…=5÷?ӋÄY`Äf@çíA·Zu@Ç=˜^?ïïÑ|^ö¿À4âµÂD3¿Èô±ë±¿à¡'A5ª\¿ç«
Û%U$¿ïúo!ËׯUNASNone3FGL J0545.6+6019?ÑÔi*ÞGk?ÃJô1¸Y?æ=1[9.?ÄX:¶©/?›Aâ^À'?›&±:b6?Áûµ<&:Á?¾Œyœ4dÈ?ç%üAÀ¥Þ?Ä@#,f ­?ÁlY¼×-Æ?¸œ¨Œý?ÕùÜǹ	?²±ÅI²%?ác
¾lY<?³¾;õ°Ž?½6í¹À?¥Ù³Š‡?Ú͛¥s¨ª?©£½Mš?Ùi£,jl/?§±^¹6…?Ǒ'^i—É?›aÃu}^?Ì.>+ß­?¾?ö)n)?çÒ#K?Àr…Û™Ó? âFéjߔ?–Ö õ©Eü?°1]³‹ôp?²ÂB Võ?éÕ
IOæX?Â_ÈÊVd?À"{@¤?»þÙú²¹%?Ók0
œ'?³Lô9ù ?â¹HS´e«?µ"Óý¥?¼ˆý.`œ?¦¬Á§p@?ÉX0¥p?¤Œñbí?àëÏ°Ô?°/	Hw>Û?Ñ|ÈUÍDŸ?¦ñ#ò ›MIXED4FGL J0545.8-0905?ïÃ4ô»À2­«ÀãŠ~À9Ó
ÙwÕúÀ;‰ùºk¡9@¥Þ^sS@Ð$ ?Àô+uúƒ?¡Ÿbûþ?ãÒácÝ @«ð¥oØ¿à~‹ì¿æõÊÝ^jo¿á>Nàð~¿äx6½¬Hs¿ã߃VR¿âñ+Pæ¢aUNASNone?îÿWtÂ/÷?"W¹nXõ¦?P'oiNë?Ds—(R¶%?Ÿ.óùÛz?"#sFY?ï¶H}›L?ƒû?Ô9Ô;?Rz@¿_S?YRr€µy?€˜žÖE ?'–Ç''~x?ì*šƒ'·?¥ç¾¦Õ}‡?ƒ˜ÕŽ¼?½?}\ºnçñl?¼81‰B'?¤ë#—Tˆ?ìûJíÌÔ?xÆ{ªj?q!§ø•·?RšñuˆE?·ŽøwÈ?Œü[a£Ôž?íO ~æ?ª]Â[M?r.ŒiG?hÑʈÿ?´`î4֕?©‰LAè{×?ï/Kƒßž?—±õÃ×~Ù?e‹¼Ì —â?rNÄF‰æ?—e%:ûh<?–*«CGú×?æ€òˆ•‡´?³lÅuhØ?•Øï
øØ?Š€š'b…?Ñ ‹þGæk?²¡Òált¦?èjQͨ?¤6iXëï?…'´P´`?qô_'Q›½?ÍÆL™Ðe?£ÿ)*-ÁAGN4FGL J0546.5-1100¿ÜÎÿ"À3U¢Æi}À:a՟Ú%{À;Þ|2€…Ì@'Áºõà@"ÕN´™?Ñh·#˜5–?âý ⣣´@|FØ+¥ ?øwÛ¿ÙþŽÑ¿{¿¸Ù"ì
"οêEœVã;¤¿ì­Z˜¿áðk¢æIv¿ïùOýnUHUNASNone?ê{zË*éÁ?¾åjtàI#?Ží2#è?'Ðî©ó,S?Ä0[ÃÜI~?½´®n¤Å?íF&\'"L?²"äs)ä?¥€î5©åT?¨Ö1yš¾?¦¬qí?£ÝÁ
Ӗá?è­ÏÆý*
?®&øµ«Ä?®ÂæÜýÎK?´¬e;S?Ř,]ð»?ªPânë2M?ävJôV:?©ÿEÕS,n?²u®«,G?•Åù~C˜T?Òv³=ã?¨8Eé.²d?æzÊÚöÂ?ç¢õýŒw?£Hjg|æÛ?¢\‡†Êµ?С^¤ÑA?'K˜@t?ç=Þ1ùø)?ÇÂBƒòð?č}Š"?Øþœ±.¿?½ÛópÐw§?·œÔޒg¹?åLÊ8üS?²3kJ"yW?· SjÊÉô?¢³;<›?Ï<­gN:B?°¨RÛ·NË?Öüñ	dz?°ãcü6™[?½´H=þµ ?§ìÝ°Â!š?àÊþsì<?³n7¯‡PMIXED4FGL J0548.6+1200?ï']ªô$À -i ­ŠÀ:3v†ojÀ;¿·lé7g@5XûC؝@³Ão1?ÏÚué‰?Ç6%ö4?ëÆxõµ#c@ú¨ïLÿb¿àóÛ>ªŠ®¿×ëD‡•¿êV¡'M¹¿éûibš)¿ï²Ô2ò›"?ÛǚþôgFUNASNone?ëðéÃíCÿ?³gwõK¨?~h¡^ÉáÎ?uõ±1/?¾''ÊÊ>'?²ð½KË;š?êñ
Ž5?¾B¬øÆû¨?rû×+ì\%?vùÐyGD-?ã÷@"Ãí?½µ¤o¿G?êȲÙ(?¨¶æØýâ¸?Ÿ—cÖ¶|÷?Qžé"?Ý𸱯1?¦S—çÑ©?îÝâɹG	?ƒ'®¼23?p[Á'˜Au?T+µë}Ê®? [>țB?'WÍîÌ+0?ç,ÿ¨û?Àîg¶6w$?‰Saðޑ?"¾4Üë"Ú?ÐÛf¾%7?ÀŸ2¤†ÌQ?äÞh"ðÁ?Ês³¸ÌK?ƒßîåhá~?"/1¸N?ÕÙøŠ¢?Ê¿[0c†?ä? Á†?²Hÿ'âd?°¨±(pPd?šÿ…lø'?ÓÍUtaâÚ?±v
~C›?ìþÚ²NØf?Ÿ®µ~ŠF+?'YfRŒ@?p/–åÄôF?µÅ?j?žDÌZ-•AGN4FGL J0550.5-4356?áÏê>€KóÀ<ÿ‹&9O­À:¯ËlÂÀ<™TÑél@@ }7Š…Õm?øàYÜë(?ÓOÎ>¼Ô1?Ïsû$y&?õÀ›€úfc@}hLðô¿é«ç¿ç4=õ.¿æ=•W¹Ë¿Â…"¿µî¿â·{ây‡U¿äkg†ø­UNASNone1FGL J0550.8-4400?ïÜÎ.:•?_ÿxŽB·?@È­ è
Š?/eOF¸H«?oÂwI×Ê?]Ë¿¶­´U?ï´%ûÎS?}+̊#YG?R⸐b‹?X[LáòÞ?€¿š2éZÑ?y[7Šæ
|?ïN<\Û±?ƒï"õ¸wÚ?hš-ºâ?e©'F¡?"%.Ä«Ä~?'¦?ïÃáhC?vÃÓ¿Þ9u?e;©Ë×4?Pü‰"" ~?›7x´³?u°¿w8—?ï­í†K?x¯øM%š?QùÓ+Æo?E#¢åB›?'EeÉã*^?w(<ð+b¹?ï¾åƒ|ø?—ùã+í²?fD*ãÁ£~?yÑH5¼Ž?›¿ñ4cŸ?•â *ž¸]?îÄ ÊI?Ý}«Ëh?q^ÅVb—?q†¯s€ï>?¡Š'&X°û?°±;¶_Y?íÉß±´?'LjÊuÅÚ?qga¨Ük?f‰#ٕ/?°¡IÕÒd?'ÃHŠJ€´AGN4FGL J0551.7+0446?é"e˜¾±À%î°t§qÉÀ9±*˜YþyÀ;…ùTTK@{"úX¡@4"Dž?ËO'ŠÝ>?á Þ'ö @w"}Š@£tvŸn›¿Á¯…,пÝ;%û'2¿ëC–ß~*¿êï/}œ
¿ð?ïÿÝe¡D‰UNASNone1FGL J0551.6+0449c?ÞlõÈTÔ)?ÆKFx=#?ÇiÄ[¿?ÁkAh;cê?ÕÞ(+9?Ãô3@ý©Â?ãӘÒ¹²?ÊÚ­"ª?Â">ñNÙ¤?¿fþ3×?Ώ_@~?Ĕ ž[`?ãlªƒ=ü?³7\Åu7?½ÓK}=(¼?¥÷¥î…'÷?ѱØóª9Ø?°‹OÆ:,9?ä3ˆ}3ÿ®?®‡ƒu–ò?Áþ39é0?¡jx"Áf³?Í3Ò×ö?§¡´!-˜?ÒIð	Îñü?Âæ£F°We?Èpzw¦ß?š}Þìκ?à¾é].âÊ?Æð@ü?ÕËôÇû_?˲÷L¿:?Õÿ!âw"?ÊräƒÍªm?Ô4êàU?ÊHe§éØ?ݟ¢ßµÕ?³B,oP™?Á¾×ãù†Œ?©á¹¥Ê÷­?ـñ.Mg´?²½‡Ðèg?Ò	
ÿ¶ÈÃ?°UíŸ?Òs›qÇ?³zÚ¢'µ?ۃßþ­Åv?³ß\ْMIXED4FGL J0551.8-2130?îUþ
ÇÀ6Yl6KìÀ;jlËÛ5EÀ<°IpŒZ@%8ZåS×@1¡šïÛ?Ñÿƒ
6?Ëàs±B?ö"ÐÜüÆ@â×P3t?î3Îc¥ÁÆ?îšcX"쌿àMªx.—¿êå"Ï7á¿È/ïÜÇ@Ç¿ïÿ~À¥L*UNASNone?ï°YU Š=?¾À
?˧?^êˆðü?^÷ó}á?€Y†ÚQQ?€!™Ç(«j?ï¥ B?"s'ݞ'?a7I?Q‹ ?pëÐùÕ^?'q%'ÑËZ?}Fq½SPi?îÎ÷Õ9Õ?Üe
	²ö?þw¢€ª?€ÀRI²©F?ž!go*#M?‹ŸŠÅ!yü?ï…kQ‡²?p	Ò—Ü?e‡‰L˄Ö?UPܝša?‰CIAA²¶?mM¹Ž"ý%?ïN3·	
'?'AŒ"!c?yMx—¸S?{õÌÍ?ÌUøg×Á?Š©'†1ÑÂ?ï¤ÍÕ5|?5ô¹Ô6?u‰àÛÎЏ?‹	\+AOÀ?˜hî
r`?•½x{NÆ[?íÊç]${é?›¶šT??'8tî²?¾¸š¸=ú?ªÍmð>.?•"Rè?ð?îŽ>pl?
`¥3
+?yÆÎ#±&?rÐtûi=<?£ã?;:yà?.Nz"ú+AGN4FGL J0552.0+2656c?ï––/ô?Çh'œ&;ÔÀ9—ž™ À;8ûefŒ&@›Ñ,Wø@[œ›¬™Q?Îb~ºÆ?Ú	{>d¿?ø¬Gõb?ò?߉=¿ØAN^²½Ø¿ß1BªŸ{¿çeQÉ oâ¿èÊ/cšÚ¿ï.mÚÚ¿ï;^g"dUNASNone(?ÐôÒL|Ê?ÃÝuÖ4Ä? vjÙQeY?¼~G%$ôù?æ~0H¶ìÕ?Ō‡s|'?ÜUÇ#â՚?Α{.ÜD?«4«CÀ=?®•¼†¬Í–?à#I#hŸ?ÌâßHOz?àq=Uÿo?²LM}º«?²úkw‡?œ‰+š"é?Ú_,§9%¢?±Öû^Ï{û?Ü.æZ›
?ºËsÿµ­?°)	7Î?–YÕKçÙ?ßÇ­ÒûSã?½^Owó"?½Xòp±%?µGD-ɕI?"çŸÍ?'Z?©4¥í£"?ë­¤³žù?¸¯xó"ö?Éðé2oO)?ÇsÔE?°j²ß?µZÈ¡Lžó?çØ]#Dž?È_bM–Ñ?ÓТ\V¿?±š$²Pšƒ?¹'
KQ"?£"Õ-›#?âô|c(Þ?²¯î›Õ?Ò聾Üt5?½›Kº,z÷?±!7m‹ñ?£ÈD
?äg˜2ÄÖè?ÁàuFå'ôMIXED4FGL J0553.5+4810?è8ðòúf—@&HƒýP"À:—Ò+ìîÀ<¾mŽxÔ@Ö!·4à@O–áXu?ǁð/¨d?FÚ
Û¢¾á?ÿ	"=—¿å Ã6iI¿æ@š>Û"¿ì¿†]|²Ù¿Î£¼ÞLù¿ïÿýF\I?ïÿÃÏÎ	
UNASNone?ïž&o)"?‡-È*Ê°?t^?ÕÒà?vüÊÿ?|Žˆ"v"Z?Ža€F"?ï ´Òžâž?£*Ãß#£?p€óRÒ?|¶±|?8Ì?—飿ž?¡oï/°ï7?í@QB#!S?¡Ë)¥éÿ¦?"Öé2‰¶?{¢zÎ.J?±»¡ô_x?žÝïö!ÎÀ?ﶣ
>`?lÆm¶=Ø?VU€†?EߌB¿?_g^ÒI?j&–E'ãr?ïoæVO†À?'e$º"î?…w´<i/?ˆ'êǶAÙ?}lazç?'ˆ¬‹µ'‹?í"<'Nîó?ºðì«~7?'¢Á–ÑÓÉ?—{èˆÞï?±	Ã8©ˆ³?¸ÜèÇÖÎ?ë"yØÍÑ?«.ïçåõ? EÙTÏÍú?•¡ñ Ïjw?¾Ì_‡­'|?§ÌÒ­Á¬¤?ï
qI³1?ŽàtÖ]ó?uGã2°§‹?mæ:.i'È?™_ÝþPçõ?Œ×U£å-AGN4FGL J0553.6+0100¿Ü ìr?‡À(¸mµ@æÀ:jíLŸÀ;¶3PdŒ@'Ù®¸»@ß	zÓõ?Ø^K¥Dóz?êCXz™@H¼¾aÏÿ?ý‡¼!ƒÞ¿Ð¯9¾èˆ•¿Ú"ã"Ê*¿è0‡‡H^>¿ï¼sÿP³?äJ
M{¿ïöÿ<
ÈUNASNone?ä	a9PÈ?Ƀ>Ÿ‰-ø?¡Î×'aÉ?žÈVBVÓ?Õ³bêD÷?ÈæGeLép?í³¦jãMÃ?¸]+.uí?˜é©»öqÔ?«
ÐmÙ0å?¨PÄrôì?²Ma'þ5?ä?:¶gä?²-êCt+È?¾
_­ÿF?§™; ¡?Ïüö‰oç?¯'d+Å¿?æþÙÊê¨?µUâ‰ÈLR?"^э˜?IC¿<'?ÐÌ_Pêˈ?´GæZ:Ôª?âÀ`Їþ?ɌȘ?©È/øæù?¦kßy²$~?×F9Õ䣃?ȯpERä?èPݓ¡?̜þϏ†?½VԄôhj?Å¿2ÛI'?¾ž¤'¾Uˆ?ÂeN-µoä?àhÒà?ÎÖ?´)ܳ¤Ò?ÅÎzAuÒ?¯M6¥¿¨Þ?ÔGP'_§l?±àœV-;?Õ¯­†zFÝ?¾ùªüB†7?ªƒ2ÒQ?«Dë&!?ã‡ÑCý}?¿ùOë-iMIXED4FGL J0553.9-5048?ê-ý¾©•ÝÀ=ˆ2¹¯æÀ:æ9ïôÀ<³ªÉlÆ@s*ÈU™º@«`¼z.?Ë{O+·=ï?¹o0'ˆ?í
Ž>F·Ÿ@S—ÖJúпä¼ò.†%I¿ã—¢^S*¿æ»ÀÖ…&¿Âf%cf×¥¿î
?¿2°V¿ï' 
UNASNone?ïȌ؄լ?kƒ'Ìóò?J³åŸL?=°ýHÜû?xc"àc?iMlž$Ÿó?ïÍEkw¥Ü?u|ܘör??F³|Å=­?RjÖ¢UØ?v†Ú«®Ù@?rf<ø<gé?ïn™'®`?<×ìL"<?kÈÓd´¿?p›ãgŠ?ˆdÐՔ?}-¿†¶8œ?ï¬yÁ?®t?baš~åÆë?aÔ4ëZ.²?HQþ6y?€l'…»÷)?`qažë
?ï›v-ƒÆÉ?xð奵?Vλjžâ2?IŽÄ'};?†H<a;L?wGÚz¤:?ïK‰aÕ¢?–0`9·Ã?_îâ òr?ze—ê°ù?"å³¢?'ZùWg?ï?X…}-?ˆò'þØ«?oymX'?rd΁ÇÝ?˜HçQ<Æu?…»R7@š5?ï*Ë®rLV?›žJ'?uh|ùuVT?f·a̒Ü?•LjøØš?{þ¤•1EAGN4FGL J0554.0-0839?éÁ¦y¦àÀ0§õƒ¥À:yB¾ÁqOÀ;ú¬ûv-"@€ÝŒb¤e@ÿñQçSa?ÊÒ¥û|¹?À–Dû\­*?ôGòø°€f?ø>3i¹×þ?ïÿ*bT3¿ÝhLðô¿ãÊGÅwÄ¿âÅaôfſ揉	ÿ]C¿ïòd6
~UNASNone?íˆ/[Râ?­—ʟî??` .?`ÞsÏÓ¹?³=Þ·Ôp?­@û…¸_Y?ïËq5ªå?™+†åŽ™ô?€'Õ…§Þ?"=ÎÑa—'?"Å'§úc?"d¡»DÆ?í±ˆ¼ZAs?œ7!V¢N?"Ω|ØÇ?€•¦l$9E?¯³Éؒ?š³1…O?é1ƒ#û ·?—(*mF<k?¢¨B•'²?|ešŠ¡d?Əì 	·?•œ[äÙé(?ìLœÝ3˜?°V=dQ³?s{Lç¹1?nåp ¼¤'?¼iAb ¯?°'2¼?í3õ›ß*?´L¯ð˜æ?œo¬çþL9?¥F<Ù%ä?®–Ê3úµ<?­°B;²?ëEßÊDK"?¨=oO­¸?•RqóÕ}µ?Œæ>	'Sn?À>2—Ï6?¦0‹"žÁ?ᐶ?¦"/Þo*"?±ÛâF?"佂¢Ÿ6?ØwSe¥É?¦Š²ªo|PAGN4FGL J0554.2-0259¿¼BñŸÈÀ,'gn¤"ŠÀ:>zt:d€À;¾G^cb¦@%ï6¯©@ys{øžã?Ám6åtÆ¿ŒÃëk0™?ÌGԪ矷?þN9Vé?É@ˆÆ¸‹¢¿àqöó4¿í¦ÉB~ª«¿âê®ñ𿑶N[,Ìg¿ãêJŒL˜UNASNone?ìFƒYç'?¸!{é,`?u³ÖÕ»é
?nPîMY³Ó?¼p§Äõþ?·ååØåw?…YNY?±%.r5?aàî1ia?lNݬŦ?‡¦]ùå?"°è?èýÃúœ®?°feþDw?>ZóZnû?"¥™-î7Ç?Ê5
e›?°'"4#?îvè6,.T?ˆA:ªŒx?W#"EЊ?Euç0<U"?§Ø`x‡Å?‡Ìæ\œ·Q?ê²ôÞ0?¼ŸóûºËî?Žms/~q?†H‹QZÐ+?ÃPа²ï?»òKÌÝë?îê»Èm—ˆ?¥µ"˜þ‹ƒ?k¸+xšï?~lÇÿ¢¸?Ÿ1…Œ†Ÿ?¤ËãWo4?æ='¸€º?³´cFy˙?–ÕåHšç?Ž‡û~Çù?Òc`n÷ý?³Ù.'·?ë8ËÌý?¥ÏÞ(ƒ›š?t\¯¬ù[?k`ø$zS?Â|ÓV:š?¥v.¬üýáAGN4FGL J0555.1+0150c¿ë…h´
RÀ'GLnm›åÀ:F¹"À;£)¼'ì&@úîãøãV@ŒT6¸ú?ÎÕ1J?á@B,Ja@Çþ0òç?øÇøâªY°¿ëL§ãß8	?ï·C[Ÿc¿à;Vƒš¿ê=sº¿ïÿýç!é¿ê]"°§UNASNone ?ФøÆ-~ò?Â-IÞµo?йG›e¬?Ävº(|ÃB?Þ¡¿žÍb?ǦŒQ­Ä?ÚÔ}ð	¬–?ÐÝ:œù?Üp¸4zl?ÎßØBKÕ?Áu"·Ï±ü?¾<G]Pç?Øl~áæ?±'Ä~?Ìúo1çÙ?¯	a6šª?ÙmÃúœ®?±Šü3´æ¼?Ǜ#Z3c?š±
~¨	q?Ø÷F´fÇ?§¦ÁYØâ¥?Û;(±`F?§Ò¶÷œ…ç?À#ݦuw?µóI#ð?Ôë—W
ó?Ço Ê˜óŠ?áç'Ê·7©?Èóª2?Ï%Ñß
õ•?Ì[qÑ塖?âõ[¸HÂx?Ð
š|K3?Å¿?ÏŒ?Âŏäšì?Í¥vŒ+X?®<_žúk?ÕœxDª?µuxC?Ü
¨A¥ª?´ô™Öçy?°°QÙöÝÁ?ŒCÔæØ®Ü?ÛÅ.R£»Ü?²‡zT§Cž?à^›Á¼ù?²`ð—àºMIXED4FGL J0557.5-4452?îS¼k3]XÀ;óìþ›{òÀ:g%¹Íì‡À<NØúØ@êç§Ä¡@t¹­6?ÂSÕÀ{ο Ş°.Ü?׍ÀÿA@špkø̅¿×@>^Šyì¿é2"²¡¨¿êÈx	&o¿â¾N"ÈQ¿ïþ
·x§²¿¶²$ÀS UNASNone?ïóî–ÃrÓ?Qق@£?A®ž÷?="¨Âtí?N—¡¼™{×?IPTQü?ïÑp½yÀ?y;¬Òÿn?HÛ8¤Sá?]šúºWh?t,:S_Žá?uˆs«;?ï]r{6pï?‡Â0D›"?d¿=…+)?d5ßV°oƒ?'Ñx® ¼?‡DiVÿÂÎ?ïé "'Ú–?JCÁÏ_?I‡•Ù×Å?5$ºN	î)?`}ø/ÿZ"?D»\ûú?ïè&p"L4?dä!­?SŽLi$-Ê?SZŠUŌ?\$Òô4iò?]:'²Ž?™?ïTfHê?¢–ªóPrž?bM>
¸–?€ ·_o'³?")"½«‹x?¡›øÚÌÞ£?îÀà,G~?"áÔîÚ?qPxR
š?r" :¼w<?¡Çî2ükF?'»©¡¿üÜ?ïµWÀ†Bz?o_ßÝ¢g[?hw˜Ö›Æ?`êçšyƒ?y'ùbq*?g*"3P›AGN4FGL J0558.1-2113?éþ"_4À4à¤ãy·|À:USʂo±À<jT¨ÎÀÃ@¿(Y@ˆœ|&Â?Ǩˆòß[?Ѓ­Ÿ
ã@÷9zu$?ýs$ºÊl?ìO"¢—D*¿ÆjOv`¿å—ö+jçտݗ|ÞÍÖ7¿ífNžHªê¿ïÿߞ¶ŽóUNASNone?íþð‰í2?Ÿ:md2?‰½ºÓSŽB?|`éíÇ?©¡ÂŒIR?™p•™xÅ5?킏Ì]³‡?ª"ƒ\8*?£}—dÉ?¢Ñn"@ž`?¤·í¿üþÅ?›ä–;Aÿ½?í,VÏÅ{?¡¡Ç'«Ç?ž¬ÞT]?'éa*¸?®5¤‰"#?š¸_Zî?ëöé‹êš?=©yx¡X?°M†AÌHÛ?‰'æՕ%õ?¯öZÎx`ž?'>
&—%?êçÉ1%«¥?²›êýÞib?¡º]¦§³´?"Š—òEDg?¿ä‡¥6–ü?°SÁåfl^?éé÷ƒ7`?½ˆ™¬Žé½?·ªê7·is?·j1ewƒ?¹Y®¢-?°à›x?ëVãñ	?¨ßóË2P²?¨(·)-"?™¼ó´ïÀ«?»ïæ|,?£epÔö´I?ç§÷w½ž(?£¬+W'?¿ÁuÚç[ˆ? ¤9èÅ?Ág5»›?—YÒ¶!ÒAGN4FGL J0558.2+0132c¿Ø%­ÚÕ_TÀ&/¢ß"xîÀ:?ûUvTÀ;¨
^u×@žÒmö} @ÉzUý?Ôæ‰ah$×?ڄKßQ‰µ@
;3Úøßz?ÿ†xÕ~Í?íµ"Ód—¿ßƒf|`΢¿ç•jËOõ¿éŽ•¹:I¿ïÿÿ>¹ú?ïc!u´UNASNone1?ã!öB?Æ!ÁEÛ?  L*é†?˜s£[xò?׸pOÚo?Åظü™?ç_û"?ÈxŒÓ&qó?ª¸¼ñù²'?²2@©Zb?ËÑ–8W?Ääe?ãVæâURË?²¶ï½Àÿà?³›ªq×S|?ž¢U6¢;?ÔkGŸ"rÉ?±ŽYMzçe?â¤1øöv?ªÍ¸¹£?¶uÍKG³?"þ²
ˆó'?Ô×Z("Gg?¨ïþ½ü?Þ§a@ÀB-?Ç|)š
á8?¢a÷ÊZ	i?ž>¢ÑFq?ß_Ç]d?ǝ×!¬E?Þ,⽋!˜?ϔe"W¶?ÈóNkÈÑ?Ċyen¼?Ø£›>ú?ÌðµǢ–?ÚÂ+–W?´\Ÿ?½¥,ä~^?¦oyÊE.?Ýøщ0Q?´¢#1¥ç?ÏîçÓ?©{—ËÅ-?ÁK»4žî?©	ñn¸]?ãêy}´%?¯é—RMIXED4FGL J0559.3+0352¿æùõ±˜À#"Š½]ÄÀ:	-ãÀ;±6½+o@µðöøš[@-¾Ý '?ÕE~ð ç?ïÿ› 'V‡@è+}\L1@¸PW†N¹?ï[Û]‰H¿¹C`Á¥–¿îFÄ	¯¬+¿ìÇæîð
¿ïٓLØ ¿èñ$?¥\pUNASNone?Ìs›)¤?ÄC²÷ì?Ædû"oð?à  ¼ŽO?ã[@ºý?Ëz"Þ³n?Ñ¡¼ëO¼"?Ê, ìcõ?Ò±û+@0Ù?ÇÎw£5àÉ?Û¬Gè]2F?ÈgY€yã?ã(Îh¶ÖI?²™‰ï…ý?½'¥½?¬çÐ#'A?ÏÚÈY(C?®+֎Ï`?ÔÄ`6÷bø?­ŽeŸ†?ÝٜF¥´?³æa×
´?ÌmŒW^-)?¦a¦ï/²§?Ä+"¨O%=?À
§W-'?ϟŠv?ȕ>MÎ?ã
S$À(Ð?ËۛÔ~¿E?ÁLÔ?Ãë­U'?ÚÙg¬Ùߧ?ÎÙîå6·2?ܞˆÎ'—?ÍHžŽdËö?Ü9¤7–š?³ö!KÀwô?ÊÆÜVòCï?²>5Kº‰@?ÖbíÉOGo?±í_"÷3Í?¶•‹yz¨-?¢iUû|f?䐀Þ.@}?»ÉÓÏWA?Ñ9›e)X?¶n‰{kÃMIXED4FGL J0600.4+4949?ïÃؐ@)ž™Ç¼Â"À:í¶ÓfDÀ<Jž6·L@ _Ž…ê:@´Å¤º_?È{T44ºó?¥S°ß¹ìÿ?Þ–¼f@Lyð'οë(øçÝÊK?ì*³Éƈ¿î\.Õ?ÆÐ{k0P¿é"3É[(E¿Þ¦ž9çWUNASNone?íÒ8ëó`?®-^ã…ä?s"úð_ò¯?‰¨u´?°4øó*áS?­"²¯Ûžy?·uÅ?…`=ôù?Q	e¥½f˜?bþëÊÀ5k?zxPÙÂ?´?'£®CÀa>?퓢{.cZ? C6Fe?	9o¤\?~jèÀü?±r›"nÝ-?Ÿ½½Øj?SÝ«J?p6ÌÍÿùß?i¤Ž,Á¾?W«5>?"2h'É­?kÀcî¡Ç?ìÃI¹œ?´!»W'°Ó?ƒÐ'‰€?‰ˆ,?·"zºMœ«?³tO]?ï<)ouP? ÅÆœÀ?i1&e/߶?ƒˆ;Ã8›?•T¸†GA?œ[ˆæ
Ӎ?ì2—zc&?¦:ìid‡?Œx'kŠ®?†aE–íTÈ?ºÜ2¿SÏ?¥›ÌÅX?îÝS»œ^?Ÿ1y˜Éð?…1†jÔ?~µ'@?™¼Å"VÉ?‡Î=ñAGN4FGL J0601.0-1016c¿ïN<»"ŽÀ/žj±NÂÀ:XÌ'©»À;žøÐ`Ö@¡di6$@
X³ö<2?ÏÇó^±ç?Ü®W+`@ü¼Ï(ǟ@Ñõ!T¹k¿Æ°(|Jÿ-¿ØiP{˜|¹¿æ£mùÞý¿ëá¬Bh°C¿ï÷íA·Zu¿éˆ²r®sUNASNone!?èç·côœ?¿ºVMÐK?"žßT{è?{¹ñã?Ë@¦ÙP?¿wZÄ5"O?7'3;?£.KAô9?ÒÝ-i±?'ȝEÔ(>?šƒø§Ùéº?œÑՕá7Å?èìëvc½?«ª—‡D?¦o`Ôº?—›ÓtuŒŽ?ÆÉ6C¢°Þ?©.óÉÀó?æ‰Ø¯6Âg?«òæŗ/?š!
Þø–?v'¼«ÄuÛ?ÑJ¬[H?«Â‡¬4»n?ãä1+àÈF?ÄÞ¯°(ɚ?–ÀLS??ÐJý?Ö˘ãCå;?ÄÇà'/±?ììíÿwo?¹!™f·q?©ø£Y$Î/?°‰à«žKR?²,FãßÐð?°ºtÞãË?ä‰%E^ÙÕ?³y•}F?±ÜÛz\	
?ž»Ú¸Ó·?Òv~–!Ù³?²x[6€œR?ÜàÍ[y3¯?¶³Þ‰¿\?¤+6¦º|Y?Œêœ>Û/?àLåè7ós?·µäÓfµeMIXED4FGL J0601.4-6057?ï1GhIj'À=|MüãÀ:ò{+‰>À<'é]ýY@¼úh;~@VÁBU&?ÓBýwºw?ÒK!{û£û?þZ%zãËí@¥Šeôül?ﱚa•œ4¿èHâA©¼¿ãtŸM ¿áà1~'ML¿ïÒŠÝ>4?êpYddIUNASNone?ï¯?[",K?vE8¡å¡?_6o"®æ?R>·8¥?€I[,è;¡?s1ïª]?ïOCCÃñ~?ŽP(š$šC?sÖï®UÀµ?x7þÒãý?'!ۜôB?†á(õ"ɇ?î‰5™¿Ú?•Ÿ¬—Èë?ŠDº–ª¬?…ÓÖzwJ? ÞŽ•>\?'KG‡.?ï
PyP_$?x²Éé—?{a¢E[r ?`N2Ü)ñ?—}ˆB¹uó?t}®Z©?ï?(®cÄå?z
Åâä?p«\¬`?eʺñÔ~R?"ð)Ñ«F?Œèyaê³?íìÎ˵º?©¤ª
Âü¸?ˆL.@€ä?'ìVgÜ+f?« ¸X_?¤ëKëu`S?í‡ã0¼`n?ž!E÷WÂ?"îê.?Œæ{‰3&?­uÉ|‡?˜-}ÙÍûÇ?í#$Qò|?•I^Û½"?"KHA§?~ ÔLÑŒ?³"
i@?"þŠ³BzAGN4FGL J0607.9-1904?ëK èá^À1쇇H^>À;-ÕctCŸÀ<Û®ïl@ b¸¬.q­?ÿ{ ÒÞ^Æ?Òâðe-VO?¾æÒ1›Ä?êÔë´ï`v@l´S"6†?ç¤ÂAÉy¿ídƒ¢·O¿â8j_oQG¿×Õ'¤´ªÂ¿ÝpĎ9ê¿ïÿ'þKÊÚUNASNone?ï®Z¾½j"?‹œ"˜½C?C®"}÷©?Oønlž.t?ƒ.ghK?Šî+hÏÒZ?ï#ª‡±?‡›aÀ›Xd?^ÀU5^?dˆí¼;ô
?"öU'õx?…¾Üoÿý?ïKAÖÓБ?†¨mL'®—?\¯'¢h?SlkSW5\?"ÌÔÂUÀ?†rà½Ý€*?î×sìƒBâ?|"<8›¢?bQAÒ??F%»áÐ
?¡c°uŒ³?|XÅO"-Ê?ï á7¦þ?˜Þ7ÌH?Y^ªi"hî?QD­,i,¤?šMîlÒÂ?˜"'Ìœ§ö?ï
£Íؙ?ŸXü[àÅ`?m$öô"qø?›KHqj?›çmŒ‹?œà–ÿ¥+?îŸ$¤5?"ncÛ¨¤þ?bˆòI¼?YO­+5§›?¤æ°Ú›?"FÉ&ÊÑ?솎Þ
É?˜Š'K¹À??sæÛIó%?eþùÖWì?ºà:½Á?˜¢m‹pLsAGN4FGL J0608.6-2305¿î£÷ŸšuÉÀ3SÐÚèÀ;LÂPrÀ<ˆœC˜E@ápÌÚ@‰ë têŽ?ыÝÄ@â?ÕHK=–
ž@¦±\.?ôV¥‹•Iÿ¿è8Eáá†î?ÌùÁâãåm¿ç=|'‡"C¿ÞùŞ…;¿¿ïÿÌ3IÙh?ïü,d1UNASNone3FGL J0608.2-2306?ï2ù@à?—@à›Yå?{U_o´"O?yaÝ<GF?™Hþ»K4?"'÷6"?îe&5õ?¨éT".7¨?"ié(ø?œœßw³æƒ?ŸóS€Ún? ¶kð³V?ì/>V§×u?¥ì†
!•G?¥1'/èҜ?™XNQšòø?³íy´µ‰?¡a©CSék?ì0#‹l҉?™9ìûÖ?£zDݳ,›?‡Ù‡Æ2~Ø?´ÁÁ7w£k?"3¦Á7}?î§þ_§?JÃ-?‡µÂãøŠ?…Ô¶êÒ
=?Ÿ%R¯VB¢?˜Â®±pàD?êËÿ-®J<?ÁZí¿ê?°Ëf\Š­^?µxŒyp?¸Ô 4K2Å?·îA›?ëy;1Ñ«¦?§¬ö{)¿?¥õ1Mˆ|™?š†¬£ë
?¹;ÉÒ}ƒ?£%ak=?åë/n¶¾?°3ÚEWäH?¶M–[­˜?¡è¤çÒøæ?ÍPxxÙþ?¬D"mÃéAGN4FGL J0609.0+2136c?ì6d}ØóÍ?ì'ÔžReþÀ9·¡I'CŠÀ;F"ôï*Æ@itû)¬w@
€™îS/?ȑ)]œhV?ØLv›gÏó@ê^ã»&?ëKÿ‡V˜¿ÓmˆÄŠ3¿â²âÀÔñß¿àJþ¥·à¿èÙÇÚñS¿ïþAÿ©ÃÞ¿ïó÷H¡YUNASNone3FGL J0609.3+2131$?Óh½ÊŒ'Ú?Ò;l›<d"?¯°:?Íè"?±—_Uy?äPvóÒJ?щ!»«V?ºÔüi?ÀwXNÿ8?È»TC=^?¿ÄJ~Ž?æJMV?Åéè«>v?ю*ù[~´?®3$ˆŠ"?ÀÌC÷ö¿?¤vÒ D…J?ãن³U?°å-Ø­G?¹"
ã12ë?"¡KiµÑ?ÒCÊ>s?ªcà ´R?ã­ú>ŸøÙ?­;ð&[Bù?Åó†ÖÁ?ÑOÝêè?²z³pŠu?³2TÉ­sñ?è3È"ÀL?ÐÄx*<:? ì†=«¸ÿ?ª…Åqü¬?Ée·X¶g?ĸêíŸ*?è—ÉÅÜB·?Ä+œëU?Á‰{>e?£¾Î|7Nš?Âr¬Sõ9l?§®êü%é?ç!ÑÉ-Rk?®%£Éä´? ´s6#@?"™CjÞO?Ó`ß
^u#?³ìÙ=r?åDNƒÆžŠ?´bu Á;OTHER4FGL J0609.0+2006¿ÎoºS‰¦?Åd†gbºµÀ9i'¹'m-À:õè½ÄM@¯r2!I@z¼i¨:?Ô;âjØ?ã]0'oí@³?…Q
9@¯upðX¿Õ1Ä{¼¿Úâ;Þ}y¿éC¿rq6¤¿ë*†ñ÷(Á¿ïÿåþÌú¿ïŒbUNASNone?Ö\Kµh¶?Èþ<öf?×à?aP
E?ÉúÖ뉦\?ÑïT
jÄ?ÄÌd
—m?·éãÕB®?´q|8…Ž'?Äڒ?)­ñ?µpŠbI?G?çÌõl0Þ?ºÆ"‰<)Q?ØÜ°ª='?µ9"Î3ê?Æ{‡‹ü?ªÓ#­H?Ü<‹Ì|p?´'u3z"?¹\3òY?"GHb2s?ÖXÿv©eÑ?ªS3šìgã?á°tÁÀK¬?ª%ô.qð?Ëó6´Ù!U?¿†CÙýœ?זì?º:?Ǫv«ØáX?Úoxfvµ?Çc'™ÄY-? ë¡ž&Å\?£¡ 2¿4?șáˆE´??À÷¥µÔF?èÊ̓«ñ‹?Á)ÌÀk8?ϬPяæ?°¬:¥h:ï?É"ÓmAˆ?¯ äj­¯?áÌ'gðK¤?´þ½ñÎË?•9&7?z‹a]îÍ?٘¤Š!ˆ?¶‹"G¡?â‹-1UQZ?¶CÀÂvXMIXED4FGL J0610.8-4911?è£ÓÍO²#À:–YòºÀ;˜=Çá¬À<Ñqk}&œ@!A'±tט?þÐæòèÀH?ÌåÚ9òÀ?q£x}…µä?«ÊD /9B@=^Wú?ï饠ÿˆ¿êŽß+t"¿äHZ!^Ÿs¿Ì‡ì]‹ÌQ¿êk[˜­
¿»€@­S8UNASNone? ×Ú?®/Fа?E˜XC)æ?g† 2ªî?‡eZXÙ8€?­W,Áõî?ï¸þx/Ur?}ܸZØqN?OȜþ&&?V;êAà(?‡°^:F›?{7éªìq?ï"‰^
–?‹äÇþ!|©?]Óóvò?dzM¸•i?™Ñ ÃšÏ?‹n®':ï?賂uãdœ?nVòÚmiN?L'&­7^þ?4ùá¼ZaÑ?"Ûp,!–à?n#™ô›o?ïó¨-Ü?•x[ØÚ&q?J¸÷T¼‡?CÈiú¹?×†qñm?•W˜á?ïVUª™
?'ÚˆE‰
?V±µ4[ø?c¦nǼuD?"ÊDK"W?'Èjò¥?î_xÂëo?–·®@?cVR÷µ?jµd²	½?¨ÓË %E?–d¨7Ö?î¿Ö,¥ƒ?Ÿ5LÙp¡?e-&¡xäÚ?Y'òsÂõÔ?¢¯ÊËzC;?ôh«cÿAGN4FGL J0611.4-4722¿ëþÔü¤´À:ÇÚÄçÀ;‹ûZu—À<¿a¥6†@ý?Ãdn?@$	å\Ë?Ó«ãH9Tµ?Äï"77y¿?îü®a|ǧ@'Góߋ@?îâ<À县ãØöT…"¿Üß|Ò¹uØ¿èDÔ «±Ÿ¿Ð6ɀ<%u¿ïÿHµ{wpUNASNone?ï¹Ão£Hf?vI#ì?P³h1O(?HvӆN]?~ñ‡11?t}"è'Ï?K¢ë¨?‰2´÷ݶn?dõÄW¨F|?p(\$w
h?ˆ{öNz?ƒ½!*"u?ï/͓ØK?†¬æúµ
?h<ÆÛÍ?l­ôý½åd?—Bgø-?…³A¨?ï}xÇù°?oØFQ?Ý?Gòl.B|?4†ŒBm?"­Bݏ?o‰O£ªü?ïP/ϕBâ?Å~`w?cÀ¼(g6?_Ô\€
À?"'wOï?Š¼uŠÈOÍ?îäü'XE£? ÛA™w?qg€"¨T±?'I)A%dî?ŸŒ¤ˆ?òòœb?îXüuS`?"‰05"ñÆ?xõŸ01Î?y'¿¬¸Ž1?§Q"Âqÿø?" ð+õÈ?î*Вmð?'lªŒÖÊ?]trÛ?T	müÂC?¬j6Z© ?'"‹«Êg¥AGN4FGL J0611.5-2918¿ìé¤lízSÀ4ñŸŒ¨À;:Z—%KÀ<¸'MKã-@O'M ð@¼ù jn3?Æ
)#ºÅ8¿"zÞåËmÉ?ÐQJ8ˆ@!SYÄAŽ¿ïÿ_Dä?ïò$	ʄ¿èL?^9Ç!¿áŸ©³`ë¿âø›AåR«¿××Àâ¯bUNASNone?ïñÑÉ-Rk?JçCµL?)ZÀŒ§qD?òèÖҗ?Y1G?·?Háú²·?ïæòÍ^å`?iWCb/"?0úQßì$?AeÝ[uY?fíè›øS?fÔ¼iÚœ?Šæ½(?':5­V1?Y=aSmÐ?`ü¤Îzz±?‹tq_öo?"¬#ż?ïܼ]á)?OTÄâ
èA?@6SÌr©?$í$0jĊ?o6àîÕO?NFµ.ãGý?ïâ¦g՞¥?bÚ¾I,ì?:ðçØws?0ª.ØcH?jz­Ñ©?ȧλ?ï­QwÊoƒ?ˆS8|ÂJ?F©kö˜óz?_i§ÿ|?ƒATô+g?‡yFs?ï9è£0àâ?‰³h¹1ç?c&™eù?hYΕá?–^uRùˆ?ˆcö›…á?y®?l‡ø=g?Täʹ?C,8P»­E?†4Êýá?k¤»É2ÑAGN4FGL J0612.6+1520c?ïÊX5ÌÁ¿õûš—À9Òc+Hƒ'À;$ý
':@jüz9'@'BÛFã?Úð¬¥åØ7?݈Vü1Q@ˆ.›
³@ŠJÇ#–?ïiGâlÇ)?Ô¿tŠ˜¿êrÇ2Y ¿í¦grÕàr¿ïüsž]M¹¿Fz•ÈSÁHUNASNone ?ç´^«ÔQ?ÅÍjè'aR? R•˜þ?žu¾æ/I?Í.0ªlЎ?ĘÁ•¿¢ö?Ó2–Ë^Ñ?đ5w;©?³§¢Í000?­N­€3õ"?ãñÀ@ï«Á?Ã?ȕ¹í?Ü:‡Á…Ç?³Ž1€'C?»Êöãž?£ÙðÄö*?ÜÒ»Csq?³¥á¦æ˜­?ÑY¦è•2à?¥—_†ô?ÑIHjÊF?­ÄõÙ??ݦÏÚ?­¡ls\V?ޑ@‹¸©?Ç:úÁ»!?¹êjŠ•ù/?´	j•ë§=?Úô$Ò>É?È5‹°«a¡?¸0`wèY?´|S'Þí?»ŽÃ_™K?·ÔQšè©?éˆi'ì?½oÉÞÓ,?ÏF9þ²?¯a$áù?')§ˆ'?«Øû"Z?ã"äžQ\?µGx­™^i?´½Â/kÒ?˜ŠŸFOò;?Òçß7Ï`?ÀyóýÏ__?ãôlxp¡u?¿i¡ÚAMIXED4FGL J0613.1+1749c¿ÚûU,=†Ú¿µ¿¿¯>-À9T*:†åÀ;dØǬÒ@ˆuÒ4j@
0'|G?Ã1U¡Îò?´Fˆ"ùª?ñÓÿü¥­@˜,J¶²"?îޏ¢ŸÒ™¿äKb¿gßb¿é¶nfÔ¿éÔ¨c`øh¿ÛÅÓ~—µ"¿è{éOºRwUNASNone$?ãC"7Õ¯J?ÆÛô?‹?z¥"Â{ûM?pYÒE
üo?ÙCA?²À?ÆŠÿwïÑ?݉'¬P¼—?θ"@f?ŒEw6 ?Ê]Í3ў?àË"úÉ4?Î1 ^oL?â
Ú}J¿¨?´ƒZ›Š"?£æÝCbaf?"<&­%?Ùmo\â·£?³ïíõL®ë?æ²dàÄ[?©ùž?…Kæ?Œ>­Ö5­ì?mÑ~³ÊR`?ѹ@Ϗ0?©Œÿæ×D]?ٌ•:Ëi1?ÂÄøW•K?q'™5è8?rϑA>5[?âúÒ]t>/?ÂÉDÍ9"0?ÐÂUèd?ÆY^·?ŒŸ•ÿR¨f?—	u»?ç,V³ý]?Æ
«,q«?Ö#$'sŸ#?³EÖ?ª¦°7Ӝ?•÷€¡óQ¾?ãNcLwå?³…4dã9?Ûjnå!=¤?³Èû+æÕæ?ÄÅhë«ÿ?†–Ÿ2š?á\¢b†î?´@UwÚMIXED4FGL J0615.9+1416?Â^4Ûпòê1ç٘À:!<ªÀ;€Uu}ZŸ@©®Œð¾Ä@sÆßî?ÒMyšöë?à/‹^¿@
9™Üµx@`¶™Y­Æ¿áOuž'§¸¿ã5­–¦ ¿âöT…"RX¿íχ\€3—¿ïþÚH¶R?ïùv
£V²UNASNone?ÑJƒ¤î??Á¿»ký)?½ÇÀ!Ýd8?¹<–ìz˜÷?ã¡Æ)M3î?ÅÖ±Œkv?ݬCtÁ??É]Àˆ$?¤–½ÆD~|?£'É•Ø?ßÁ
§2?Ǽ‹)FþË?Ûøë¥(Õ?²ô—##›?¸è1©²? Fr̘wð?ÝãO,…f~?²ê³•'ËÊ?àÆљ¡bw?°	Ádн?µ¶ýŠ˜Ú?•Úhh_•?ٝ‡ÿ'?­»ô¢Ô«¾?½±¬F*ÂÝ?³ÏANÝfV?ÁVˆó?ºÍUÉ5=¤?è†â µÇ?ž#']£?Ãz<F­8ˆ?ÁJÁ9›­?­š¤xÉ)$?­©aYS†Ï?éGƦÿ?Áüox=\?ËÅf;ž;À?­%ª1*?½A™¬¨®Ï?¤´'ä.?åfs:ùê×?²-ÀOãX…?ɏ_»É¼™?©tÍXúZ?À(‰ê'Ý?§ûޕ¢Ü?å'–öYÂ?°Q¢c[ˆ×MIXED4FGL J0616.5+2235?ì"JJZ@=õ~œ¾À7ÈE`\a*À9ÞÅFƍî@"ϝ"úh@R¢™ó[­?¸–¾»<,?¬ø@¡Žc8@ÂJ»5'@V¸­¿ïâ'x?܃ÒÝÝì/?ï^ˆ¶óF´¿Ú%р´¿â#πÜ3¿â"@^"àÍUNASNone?ªn4"âÒ?¤ÿ!¡¤û®?vùó÷^è?xY=ºqê¢?î+#$¥ÚM?¦ñ4?ߖíÍxnQ?Ò>ã#Àn?¦wí9ŽH?²
k¿›ÕÂ?ݦã4©f'?Ñ6b™
"Î?ÉÝašy¾]?°vՓRª?®Ž´ãFíÂ?¡'äsÓ#?矼Kc?² '¢?¹bµQ"`?¡Ì/]Ó?"W…4H?†!µ?Q•?ì9@³4±?£ô¶ÒÌŸ?±UŽÅ?«ÕîéÀ$?uÒ:Ò\?vP|ÎÁq_?í©©É´áÁ?­+´uA?Ô%‰	‡ï?Ï]ØìHp»?±H>û®Û¢?¾¸û3½q»?ãÄ3›¸Ø¤?Îєݝ)œ?Æj•—+´?±¸ðE#«?¦¼|Ûca¦?žÍéú§s?èù'ïöy?²ËüE¶?©Pi¾¤YÖ?™P±
ˆöÝ?—6i0‹²?"¤+ÇBÅ?í®°•<E?¡™Ù]éeMIXED4FGL J0617.6-4028¿îø`ÌQÀ7Kğס<À:Y:Ütà}À<Aß®Pá@"ÁlFz8@²c/
°?Àâ2d¬'¿~9¡æܐ?´Œ•z%5@¿ê»Ë?èQ­DqI¿ã–ñH­¿éŸK¿ñò÷¿í-­LÔÄé¿ášß÷-É¿ïýVlô!UNASNone?ïûÔNmß?7â‰^›‰‡?"ôië©(,? W¯AwŽ,?7ãYL*?3g¿}!]?ïéVPÇ!?rHFêF?0•¹þùÇ?C'=þ÷?d—ÓKaÀ?pþúX?ïU"`?‹-i¹O?_¾€Êët?jˆa¢Ú"‡?"_Ëô^ÿ?Šƒ±…0œy?ï÷@KA?4Ñê‹?e¯9ĵP?®PΆ,?Pi|]Qˆ?3F82Á|?ïùø1)˜«?B˜ÌM…¹?0ŒÞ-±j?.땣‡??²uÁ¡Ã-?==
˜VJ²?︇Jâ|a?QšÜ¢žI?CHï#áB?[Úíñ8}§?€©žXŸñ#?ŒF"û)u}?î°øî
V"?–Ÿ¹p4?hˆá%Jm‡?oÀ^Q""?£gã
ž6?–Cu9Å¬?ïä§ý.?V7<¥H^Ÿ?2¶úîr¤?%Ò±èHœº?i™yÊWÂ?U)µë½³iAGN4FGL J0618.7+1211¿ì¤‹t¬"¿ùvœ>ˆÀ9Žé#D¨¦À;G5>¦-ý@ʈzdØ@5½ÿªo«?ο<"÷?Øwîý`h@ëð«Ï?ýÏôÄã¿ÒÁÞݢĿâT‡@сg¿ê±  œX¿ïþ†¸ìE8¿î{qZ¶.ü?Þ>;Ú¡¡¦UNASNone?à[ÛO"Þf?ɸµW?ˆÏœç«/?ã´™Éðò?ށÌyÑäJ?ÈÑlÀXÜK?àÁ®¸("¸?ÈïvŠ©o?¥4ąe?£Ê'2´X?ÛÖ	ÿT«Ë?ǵ‡ƒ—z?âÿ…N^ñ?´Ï6xPã?­ùÛìç?˜cdIÛp?ÖAÑèPÈ?³6j(ËwÎ?᪎?Y˜^?±÷è¡*á?²l£Ò ¬o?'Ï4¥ê?غŒr-‰?±å›Ìa³?Ó:d©¼–8?ÅpA©C—?‹eA §W'?'÷33k?åõ8¦º"f?ňä¢xݯ?Ȧ¼ô"ã@?Ä2^æ¯?¯»ý-Óýâ?±5µÈP²?çڐð'ÅÂ?Å>ºQu?×].j‡Äk?´›ùÛ5¶¿?³<ÙO<(?œeÉ¿nmÛ?áßa/M~?µKn	ÔÝ?Г¶Ø¼´?±ùÐ¥«h?¼Dµf©­8?¤p§>2¸?ä-æÌÁÿ?µÆ@tAùÓMIXED4FGL J0618.9+2240c?ég"*GYä@díoڃoÀ8£$G%ŽÀ:V>hñ["@ä-;¢m@0;>šo'?υŠX‰?×E$>MÄ@h›€úfc@ØçÓ
ƒ¡¿ìŠÝ"3¿Ù_`"T"«¿Ò'¾+I¿æO_žÌ'¿ëá'fw-^¿êœöElUNASNone4?©XÜæ(D?¢uÁ9?ǕnžT{?Á€JGÖ-?è….$wûÜ?Ã/©]Se?ÀµÃéؖ?¿ª"Ö¥Ø[?×F[󵈧?Ê­oÜ©02?à/aޅ‡?Çúk>?¼$á>|?£¼)°`W?Ës‹¤¾î?®YϪ!Ò
?å ìñÒ¸?±F	FŠ.ì?¦Ì^vÂz?"Äžsçç?Ä·˜*Ѳ?£["/+?éeYu ü?¤#¥nÀÑ?–ô/?ŒýeâV"¬?Åç®Å¥¼?Á«{Œpïµ?éÑ+¶è	?ÂAB9$R´?¤+T8×?«‡få›Å?ݳø&å?όÉOra¥?ßƝG<ï8?Íè/¬!?±ˆØN‡¸Ì?›û8d(?φF¡?²hÎA¡Gÿ?åíSs"?#?³*²¼Buw?†@ÿ	òx?nÑ5	rª¢?Ç2Ô7>?¯Äù¶é?éÚFö°S?®ü{$ß>‡OTHER4FGL J0620.1+2246?èÁ÷îRrW@
º"¹À9W|i+À:ðÁëÈ:—@!`>Æ4W@F$<jÿ?ÄK©â,£?°Ø*ùÓÁ?óR¥ôñ¯?öí՚¦µ¿ïðÏ«¤^?ïÿ}ÄPýI¿è¦,Od¿àcuÏ¿ì×LbY;†¿±²à<–3^UNASNone?É;`¢Æر?Ãàmy¼@?‡"£n7I?'Ó¤æR|ž?éT©"À÷?ÃqÓÞlv?ҁ_~É<R?Èþ5Ÿ
Í?Á>'­‰]?À‹6ns?âo«Õ9
–?ȤLâ?×jŒ.ˆ?³r¢¹ò¸@?µ0Õ¡¤ÙR?¢Ø‡të?áÍ0>%'?³hT¾æ]¬?ÍýÄ;ƒº?¢²Ø#Õã›?»¾2ïÛ3‡?Ÿ×?"œæj?åD:0õ¸¡?§%ēJþŠ?½E´ù$!?´Âc`yFÑ?'£uzáó?¡òùE?ëÂC¼˜L=?·¯RBHù?À&od€¡ë?¿1xf Îà?Ç&x—*Ô?Ç=rÐ	˹?æ,Æ zÐ?ÇØÔ?æR?ÌjÜå:q?®
7)šª§?·-öÞCB?¤)ìý2´ø?æCÞèû?±p~'AEA?¶øaÿÑf?™ªÄÎÌba?ÀóYž¬ÓÞ?­áhÆåú?èäXÖZë?¯ÎQ>-"•OTHER4FGL J0620.4+1445?¦ðÊ¥L¢'?l`ÃËW"À9ªu߀-¸À;LM++ýµ@¸¹Å^@F&}BJþ?Åʤ¾æ°#?¼X̔m¶?÷pd·9½'@´Áº ,?ïÌÝÉtR¸¿ã¡fµN+¿è=Ëݹ"¿ç_™Ã‹«¿ãË£l2›¿ïÿ!}ÿ	`UNASNone?ê~æ'Ì?´E<©A?hxx!zÕ-?^œn»,»?Å¢†ïÜz?´‹ô?áf‰µ²B?έïÅ~?…cþ!ñ{à?‹S&#™ý?܇̣ÃO\?͜ ¥šŒf?êÃٜû	1?§h¡W'³Ø?'¸ÔJÚ¾?ƒËÂA‡?¹&ŒB?¥üÁ¼`^‰?êÎnk©­t?—·ãÉBª?‡;íÑ}?bÕ%	?ÃR‡v×LØ?–ꍑžY?â¸gu¸œr?ÁP$\Φ?w£2¡–ª?h¸Sžƒ¨\?Ú0¤Ôqm?Á;/Ä
?Õ¢L8ÆMµ?ÉèZiOq?‰HoêÐl4?—ú #(Q—?äɸ$
T?É&¯)?âËÕ+?¶&íœÔv?¤ŸW(ç¡?'Žê±<¸?ÙE󃉦¡?µiDª8?ãÓGç0Œv?©¸«÷?›/VxÀWµ?~6˜»Î(?Ö¦zÉÛçÙ?©BŠ¹ãÙ1MIXED4FGL J0620.7-5034?×®NŠ°%UÀ9Q—ÃքÀ;•æR¯Ð=À<ä1Uãad@!s?Lœì?³IWaæ¤å?âøVCæ?ï÷q@ŠØ?øAÔ¶¦@J=g>¨‡¿ïùæÁ²À?ï}4ßݵ¿ëG¾Ûr'¿ÏkZXæ÷¿ÓkÁ¹É:¿é)g7F¾*UNASNone?ïg»Ú|Ê?¤jOõ£À?LÈQ§°ˆj?P÷
ˆÑ®?'"B.ª‹¥?¤5ɝdÌ«?ïˑAÓ?"³ÜòÑò?KÔå#?e	 áa,^?vÔÿå7?ÓƘ՝?îT±âÝý™?!ƌ1uE?{¬3Ï	Bí?G ln?§?[USS?›oShëxu?ïEf㨠7?†Á<ÔOU±?6ÐБòaL?:ƒ32:;?–÷àDûfü?†±uªèP«?ï%Î(Ëü?¥¸ZW—õ?c4RMmܨ?d"Rº'Ò?˜ß°—F‰û?¥L@EK€à?ïUÎüQõ–?¡0úZ	òÙ?iàçèÖÿ?‹ó¤ä¿?'
™OU?™ƒe9õØ?í¸qô9"`?¢(²†?~c­®_^?"à‰'ët?°DŠ$òØÄ? ða¼Þm3?îß«ñ#Ýï?š'úKBñ?+Ò_*á•?@D§TÞ?¡én'0£õ?š'
¼ôAGN4FGL J0620.9+2201?¾¬úý°@/ !·"À:íFƒrèÀ<º&‰@$d/€ KÐ?ø÷3"«C?Ǽõ©ºÎó¿ŸÔ€Âªk?ÕQÓ1jÜ@Vô²ný¿ïÏJöžWn¿ÐÐM_Ú08?ïývþ«¿èÁ€}éºÄ¿Ì"O
TAÌ?±£až²UNASNone?â—ȨÈ-"?ÍÔ«9:oy?Q‡u,5hÇ?NgŽÆ3*ý?Ú¾ç9"'B?ÍÑ/n=Ük?åXᢿ)˜?Ќ€hΩ?}'ŸpóY?‹DêÜ%‡?Ô×ò=RNŠ?ÐR²f¼nþ?çr­´%-ƒ?µ7'²©3?h)Òc?lU÷ÒÉÇ?Ðé"D W?µŽ'æˆF?ìP—·c¦e?¤ðû=>?MÑGÛM<é?E£²Ol7:?½?Ÿµ	+?¤ˆ0}§?ãjìåäÔ?Éõ¸Sn+?`ÅN)ø?V™
 ,%è?Ù
	Y×?Éë>)'ãì?ßɱ´î^Ã?ÐE{$8™z?}ô+˜Ú‹ã?'ºéFrY?ß¾}œÁtÞ?вE•"?眣Ÿ
?°Ö<ÚsK?wi'J‰öÂ?ucg;úX?Ðj9˜Ì¡?°³
,Iw?æ&\4b³?»%ÐÁo¡?\Áó™Wû?`™ÇæX?Ӗ†"ž?»4tfYPSAGN4FGL J0622.5+3120?íV°ó
²@ K£ÂˆÀ:*3°1À;»©É'†@¦",0‹@žÜ~ñw§?Ñ`šŸ~
?妟Ԝ$@âZÛGº@ÉîvÚ?ïÛ·`Ô×?åå[¤k"³¿ã¸¥bûwÛ¿í͂iÒ+±¿î
^þ"¿ïý'AŽ?ÉUNASNone?Ø°9<¡`?Æ:àC2@?®ð|"õ!?«^eîŸÄý?áÇ$lÏi¾?ÆÌ>߆/Q?Ò{‰+jx?ÆçÂEU?Ö´Ï	èâ?ÆT'²ÕŒ?Öϧv볇?ÃF'V±°?âfM'Ù1?±—:‡7Ï?ÁßÓë"Ñ?¦Ð™ûqÙ?ÒÛ¨z惶?®4f¡æp?ÜZmZÕ?¬p?½Œe?Õ\^G*ƒY?¯£VÖ­Iš?̓fÐC¥?£ÊSؑžp?Í÷sML?¿\Ð܍?Á©ãÇBÒÁ?¹Wð™B?äÃñ[øN?ć¹kཉ?Ãc*‰ˆÍ?"ÎGûO?۔§"¨
?Ë|ÕÂÙr¼?Ú¹Ãi»tO?ÉN_¢R?ÙjV"¦¤?°ÜµS.\?ÊÊZq³C?®L(=/<?Ù0|_!"º?±hšÌ‹?ÌÚð€J?«sˆ´€6?ܾÎC¼º¨?¹
S8]ÕÎ?ÔÓ¹|DË?³29ˆ€ÐGMIXED4FGL J0624.7-4903?îؑԩ:!À8U»YÝÁèÀ:Õ}<kÁÀ<…´Eâb@òàY@@×Or.Å?Ð^Wú?ÔXsÉü7ô?þø_<¦y|?ÿÃVçmb¿âC"×ü¿Ü·ØIё¿ç›ÁýeñÌ¿çè"M×ú'¿ð?ïþª*
•…UNASNone?ï0?­ñ¼? 3ˆÕ'sT?r¬™wrÏ?mÐ7>Fhð?•Lä,ý'?Ÿ§'@k1?ïN"":?'jŒÇô?vøÂ|ÿ?ÈÃHÙ©?p#¯µú?‰2ö±Ôw1?ì¯%Á?¤ÒÓê%â¸?¤­W*xz?›c_¸Ü±Æ?°1#'ì8?žÉ_êRB?ïJbðmÄ\?w~<rTaÓ?xìý»u ?a'cêW™'?xb†?Ç,?rEˆÆÅÍ?îÏƧCÑ;?¡è[¬Le?|c˜¡?|3±…ŽÙ?žîED±? øÊ>˜1?íÊekŒ‹?¯5P™)ð?'"©Ç:ò?_‡ßcÒ?ªÕ—õË5Ø?¦öGcÖd?ëúÐÛq¢§?¥ù÷¼j­?£õ—7Â¥?™ÕwÑDl?¶.­^×s?¡Ð'è;ãè?íæ#z¿ ?•I½ŠÐÙ?ŽË;I¤†)?~½JòK'?©ä^ø~™s?'Wy¾¦ÒAGN4FGL J0625.5+7029?íy[bɛ6@7Y±ú¹o"À;ªçä€G¹À=µj°x@!jÄ@?ú±´"#˜?Ô;CMÄ?ÊI¢¶MÚS?õ‹Íþûô@‹=8ÌÛ¿ïÿâÙ~‹÷?ïÿúŒ—Ó¿èÞ*o¿yî葵†¿à]½Ž–[¿åª[Þ£
UNASNone?ïϕl8br?Ÿl¹éO¢E?H(9Ëà?c–>œ¤?u0B՟ÿ™?
ã°]
?ïÒýחè%?sðß;ö¹?I
§•K?S"äs™ç?s_¿J† "?p¢­¡ÞÁ}?ïځZ!x?\–š:ó)?tL·ÊL`÷?zºþȬó?š1â€®µ?GKôE?VW?kŒ¤ºqB?g~\Á¿Û?Qj;|?"TJÂâa`?ioÈ­µÝ«?ïÁÕùNé{?—s ÌîϏ?U˸öº0?tˆ|{|©C?yÍPv¬,?'ŠÔ‰ùvK?ïyÅ?~‰ã?‹»Mä(?^Ó²>^?j8éÀs?´9Ø黛?ˆwâ»PÂ?îsCûµ÷?•ŸŠ¢Åb+?|üWKbÌ?~	¾‰)í4?¥B¬6¥µ?"v''[?îêã?†ÚïÄ+e?x6—
œ¤}?o†Ç©?œ¢xñð?…Uö@^uôAGN4FGL J0631.0+5626¿©­A
D#1@3¥õß덂À;-DÏ<é•À<ÁŽêéîF@çÁÑ;?ÿúü‹z?ÑaæåQÓÝ?ӗ­µ°@Á[šZ‰¹?þ²Í‡²¼U¿ïàîzÔ]?ïF"y&²?̃K쓿Þ>˜â9›'¿é6Í0ŸÛ¿ïÿúŒ—ÓUNASNone?ïb¸s›Ðx?"Cºjû›Ÿ?€Skÿ®Õ?u
ê¡n ?‡P¬´=/?yÞ?›‹^0?ï"KN‰?™¸ ì]?…jŒ4t?‹ß—Í(e?"p'U!ž?Œá"«%&8?îЂ›o?']Ðe"¡'?ˆô×E?"¥çt‡«?›`å?Â…?ŠŒú©ó¼¢?í¸BŠ‹?‡úÎ@Sýå?žk'­éž?ÊÅõcã?¥IB}ÎÃå?~ÄÌîȯŽ?î†nŒ$»÷?—Õou¾$?"Óa×Ús´?Š8yùS.?š^Ì£Ž
j?ŽdD¶ÿæ?íwW3‡ZÂ?°«vØ!à=?G:ò²I?¥vÓ_n«?ªé,¤¯¿?£Œ'	J?í¸ÏŠŸß7?œzØõ`P?•lN^'Ž?Žóº!ywe?©¼à'"æÏ?•3RzZn?ëŒ+{žü? ?Dò?§¸y?ÈG ?"Û–EÁ©?·Âg	#?—ÛÁ¼‹Q¦AGN4FGL J0632.7+1215?Ú1{U¿X?÷¦Kç_À:
á'ï¤À;†}=B€®@"'Ñÿ;µ@&eÅV·?Ëc¬¢µÍ?Ô
"þLf@	"•á~4¹@ƒwçî¿»Tÿá¢ô¿Ïxbmοæn'¾-øŒ¿ågµñ¾ô¿ïÿþˆ0»Š¿Ì<Vžó UNASNone?ÕaA;W?ÀÝü¦js¢?®%òÖë—?¤á¨?éi?ãm$_þÜ?Á›dÄi•µ?á³J(ÜÜÔ?Ìqqtþ"?«Lº¿½?¥;}ߝ›?Ù/ÔkIŸ?Ên‰]êÊl?ßԝ|?´ˆ‡Ü)w?²	mïa?› Ï{¥S?Üci›=øM?³§*$EÜ?å/9µ>¡â?¤:SÉmy?²bËU*3B?‡w;¼<Þb?ÑÙÀ²‹?¢™¬_7í?ÆMÌ°?µ›Ýühÿo?¶K®?0&?®×*©èÖ?ç£Hó ?¼–!¿îB?ÑÃ+ÀÅyê?É[Šlwnï?¸ÚT$^J?¸Ÿ¤«³‡?äæ@¢?Ê`Eå"T?Лƕ%@¬?°µ¾ø5Í?¸,æ? «¯"€÷?䬜Sc÷?³>éѓ§?×°½lÝxì?«F"	>·?À½iÛp?œ-5~s?ßðµ^5\?®Ë~ïÏOAMIXED4FGL J0633.9+5840?ì;™)mj@4¾™A…ŽÀ;dûHábÀ<Õ±·Ÿ@ 	ËÚŸŒ@ÎÓš3ó?ŧ`Ÿý·?À­ëÇJ?ÂQœÀ? ª@ñ,}ŒrÀ?ïÈW¢~D©¿àW@Žeˆñ¿ä t´Ý¾¿á I·6ì¿ß‰ˆª^ü¿Ô´4iq3UNASNone?ïÌ	¾ù-1?fúvr/ð?I^Ӛ,?87`l«"?vÏF)õ¯?d1øQá ?àc­?ˆg¦Dü?d‡µèðôé?icœcγŽ?ŠØ§ü|Ë?…G2Š?ïi8"ÍÛH?}§ª˜NÔ?b±žÓ»ý?^FxBÝy[?'¹º=¬s?{ý ªÞÿ?°@?gð‹ÈP?b¦üoXþ¡?DÛNMËyã?†/{jDòl?g²Ní‡X?0¯?y&;ŒÏc?X™ì‡s˜?JtûR¼?…ÓŒéä³ê?w€1必¼?î×K›´ÑÙ?ŸsÂR+Ž?p‰rÃã?xìÜt¦Q? ‡•Dhy?:úƽæ–?îæØ èØÇ?Š(®ÖßΜ?j—ù¿Ê´Ý?^ñçmÊÏ@?ŸÑü²N¹z?‰—ÿÐ*0?î'+VÎvy?†"X÷bن?|BéUaåÝ?hkqþùx?£díl3í´?†èßT"õAGN4FGL J0634.6-3046c?é¨"EÐÝÀ0Ï8£µ|NÀ:8WšÀ<DOúêŠ@¶Ñ"@ÈòZ%"?ÃyR¼»\¸?׏=Ë·?õ#ºð+w@qµ_ðý¿¾²»(µ€Ö¿å«;þ/¿ì¥• æ"õ¿àê¢Àß®§¿ê˾ßK¿ïÿøÞ£ŽæUNASNone ?*#¦4?ƒ§:åVÍì?wÇ!g&?xO[ªò¾?yëY°˜Š5?utùDƒ¡b?ï¯õiV¹S?ƒ»s=?`҅Âxë6?k‡0תs¡?œ'S\Ò?€‹E—Ž?î˜EÊB6?•¹'J\?…z}~î¹?ƒßSÈ4"Ñ?¡7D» ôe?'Ò‹Õ@ È?ïyÖkî!?kõÀí¸?xa%q¶?]DuVe?ƒp÷ã˜Ä?c}ø1·)?ï'¬\È`Š?'#í¸-B(?ŒÑ°8 ì?ˆVo²Ç;^?ŠñL¤?ƒ@€ø¶|?îðìá.?¡*üx¤?€˜´‹E?'?'ªµ§•{j?™–	š—?šw'Ùr&Ø?턔9ù1?žšuÍ/?"¹–Jjî?•B±{Cµ?­ªá"ªÓp?˜ñ1tÛãÛ?î"ÝÃr¹?Š–ƒ…H8Z?""_FW?f?Y}s?™ïèDrVÒ?9Oå@*AGN4FGL J0640.9-5204¿ì]9ů³HÀ6Ÿ(ǟfbÀ;Ì
V)ØAÀ<ê?ÉC«P@ Éí
4?þáÁçâÓ?ÛÚ-þ•ò›?²ÞÐZuíB?ÚÂÑ84$@	Î{"¶
¿ïü3ŒõFi?ïþ^‡tÔ¿çQ°''¾¿â?bžÍ¶¿V"ì"q¿ðUNASNone?ïßR-tWk?ž1{ÌIÝ?;ñ"úV&Á?nõR¸)/?m/®2ö©í?š»­˔?ï݋ŸÂ
è?uшXáý?7~6Gû
•?Më³×{|C?o"™?Ÿ,Í?sÔ·?î®qýô7?˜¥Íõå̂?`TŽˆ}—L?qHï¦J:ä?¤—7nË?˜wÅ»3èÓ?ïäœv?Tœ?8<™?3Ù²q[?
£Ð'Ðó?kK[‹K
?SóӖ|n?ïÜEKú?Q——ùÀÓ?>^·q½i?[%1<3õ?oéóÓ'?šr3X"í?ç{û?u@E€ÂÒ?I¼¢'Nt?cŸ.ˆnn?†>­ÒÆñ?[™¾3€?휊j&ºT?¢È…Ç(Ü?i]!ñzØ?wk²@žF?²S)Ç\r?¢´qBT¼¯?ï§pÝÁDa?tÊÕÇ__?#±;9ëæ1?*µÇâ趫?…Õ©¸´?t¿è8::ƒAGN4FGL J0642.4+1048?Õÿ…)R½E@{XÑRm‹À9ïL}‡\À;'Z5Ö{¢@‡åÇÅ{ö@F¿Ä§?ɐ]b²?ÖIí{ì
@>)#øÁ@TbCÁö°?ïä©B."Ó¿ßÄøÂôܶ¿é¼O§@¿çòáԛÎ'¿ïÿùSt?ïø#ÝÕ³¦UNASNone?ë0G'Þ?·cD/{¦?'c_d®D:?ªA«²k?Á'Òö1 ?¶+°
ˆë?é*µ=í~ý?Åì*ڍï[?˜àÂÝf¡??ßۖjðL?È9¬f6&?ÃéíˆQ?éŠðsx¦?¯
"B{?žKŽ¥ÿr?'ÁÆю'$?ÆŠkm%6?¬ÔTåçNN?ì8¾±ðÂ9?›¥ï@Ô¬K?'fƒv?röŒ¶Ÿ W?¹ÖÆWµ?™Tžˆƒ×?æ­æD
?Á¤—à̉?£/]Ñòp? ѳø{¸?ÐA.^¶w?ÀÀ Ôyû?áS4ÜðJD?Ð6`Ý̋?®:%ø"'þ?¶há‰h<?ْQ†…j¹?ÎLó[›?ä8+ðɬ1?µ^ÓüR1·?«û°Áғ?˜ª@Pæ?Ô.(¨¦ãë?´£l"É?å~•(¾?²{Lð>‰?¨ë†or?yEZ4üL?Ò£'÷<¯?±Á@6šÔAGN4FGL J0642.9-6501?Ì"1°Hª
À9L[9âyÝÀ:‹¾‰=+À<gñx7@qGÛ
þ@¬ÂPr[?È«k=»¢X?²6ÊA'+i?ãEºßd@Ù¢.¾"`¿àûs¾¾—*¿âº›aÅ¿çvx݌b¤¿ã'eMa²¢¿ïÿ¾&@Üi?Á#%^‰MFUNASNone?ïÄH=þµ ?š\ɕÆâc?Qï.?é-
?B©m]??y`y™àð?šZÐ8Å¡é?ï³Èk¶~Ï?}Gheµ‹?Vܗ'žß?]€¾÷5!é?€Ji';^?xÙ7 GŒ?ïlºðE;¸?~œÉBâOV?h%9ò~Zù?c׈ÒËä?ŽÇõ|¸E(?{£;ޚV
?ïŸþ!¥äx?aðP2'Œ?c‹Õo:>?E'îØoÎS?ƒ'a	«^?^Òä
Q?KóE?†$ù'¬hê?b7yG£Zs?TgèøÂî?‰Î³›'1?…Im,4X¦?ïE2["H?–^KD3ý?h+™RJa?t\ t÷D?™'æ"ÊMÃ?"c'H—"?îùÅ¡½Ýú?‰hHX׿?r;f3—?j×.ވ4?œEFxbÑ×?†z8 K?îèÝá¿oŽ?'#Eö?z¿íIO?f†¦QRÎ?œ_Q»tæ?Â7ٜO=AGN4FGL J0648.6-3623?ã%'ƒLÀ07jøœ^pÀ:ÐrûÀ<A5" ¼8@û˜‰y:ÿ@ù—"ÆÔe?ÕGwB¬¢á?Ö~<ЕÚ@Þò"z–@%xÄ¥?ïgF€l÷пã"E	Œ³¿å/Gì'Ü¿ê;ÔÂd"¿á—½¡`¸R¿ïÿþó…õUNASNone?ïdÙýü‰m?'Gà'7É?bX<Qößô?VŒèÌ«Áo?'¸µTk?€øûZ#?ï{±(g¹?çƒ¹0ÙT?oµårÍ?uwÌ>®MÈ?‰MQðÍ,û?ˆ_¤§(_?î`¨îß?••»^S?l'ûDÚP?‡è á+,?¢šLSâø€?¿"å­n?îÁæfË®?{&cÇ»Š?xÊHŸï0?]¯˜Â*ȱ? ÈP…0»?xó^>Ì.ò?îk³íû?Ÿê›vÞä?rq~•æ?n"•'êÁ?§dð=Áâ?ž)»Ó9Õ7?îk""Ä?¨˜´<ö?‹pJˆñ?š†k[ÇÄ?¢€c¶µh•?¡¯ô´NO?ì²B‹ˆ…?¢îÐHP}{?œÎU³Ï–?'UJ¥¹º+?³:VC"»u?Gyèم³?ìðÒñ²'í?•SàpÑJ÷?"µJÚV¾¢?vóN2gW?µâ¿üwÀ?"×òݽëAGN4FGL J0650.2-5144¿ê±4ÝF0€À5'	"ãÿïÀ:â$GÝå#À<ž¡ü>ª`@!N
©§-×?øñ¤óið?ҋ‹#ŠÑ?Í5Táä·?û±¾‰=+@†+ëÁ.´?ïúöv'"¿íx¾W¿¿×ÉA|¢¿×Û;Û"zÿ¿Ý;ƒ"…F¿Øƪß<;UNASNone?ï'éÂ%ÿÄ?›	p.JÇù?N>æ@n®Ï?fË}ª˜J?‰¡¡ðøR?˜`û\FÓ?ïm®·Á€?‹^³Ez#?eýEc€
È?m6
‹n½‰?Š%Bü÷.m?ˆq{=D o?îà/> ¾k?'WÅ̘î{?gõŽ\+©?h'œD£®Õ? Œ¼»'ƒ›?'Ìr¨Ìº?íµñÚ?‰•ìœy]?qÕø
Nt?Xn¦ŠüÇ?±9È#e?‰#ûî߂m?îêÏö33Å?š×@"RÖ?`Œ×>–Å?V¯ŸË¥ðì? J?ΨîA?š<í'ô?Ìï~Ë?¡Ø1';ïu?w2)Å?…xæÞ«Mt?¡Q¬µ%? 4rž9.?íæÓQÔ½?šTӖëip?l¸Ç* 7÷?m×ʯ¼³?¯Ô6WÓ¹?šïÇQ!?éªõµ+ú?¤c'O'?~d{"EÓ¼?r"ÌmŠQ½?Èd¬M·?¤‰Dš‡ØAGN4FGL J0651.9-4330¿ÐZü$ÿÀ24GñQçÀ:Ò¢ªºSNÀ<K Ÿ²¸@¶å‹Š7@jUp
?ÖĶv$J?â³7É
û?ýDr‹7×@
M"¿ä|m¾I|¿Ñ!åBq£¿è%–ýÝæÑ¿ïö¶?¯?îœÏä¯A¢¿Ëg!!bÑ1UNASNone?ï·à.9?§I[¼õÛ?`!] ®'›?z"Ú?|`áqÍ?¤7'Oàné?ï_ð;D'D?¡4¬e;R˜?v¯ŸêqÈ?‰!Ue7<W?Œ¬cÏK?œ]Tã¿Õ?îBšG&Û?—üŸxUÒ?Œg‹–á?…Ø
_Ép?¤¼—Žf/–?"ÑÁXncÝ?︛õ¿_Q?q¾ãý)YÀ?0DûQ+??0ÃcoÅò?VÚ»£ˆÉ?qf¬Ž"/?w€	?X?/‹uú?qVU<Ó´?|rh­´rÕ?…èxxyÉ?‡,5r??îz™{^¦?±2Îu£®?Œ¤ôÖ%?¢rp5Í5`?¡2?
ú?§jÏ=Öªe?ìyÔñù?¢ûPêdsƒ?›K'a©ú?'ýV1®Üs?´AnŒßþ¬?Ÿƒ™¢ßÛ¡?î Üw~€?›]\4ZæÜ?V°ë?µ"Ð?ayý'Ó?¥J*àB9O?š¤´47…¡AGN4FGL J0652.8-1855¿è>ö«¡±À jÑÐAÌSÀ:¤V¦ÖÀ;¬ƒ•KV@@™vÈß,v@±«Vç?Î3[!8ßÅ?ÇFM^;J?÷b¢Œ‡b_@¯ãËh?ïÛ †ó¥¿äÒ¬9¯N¿äÕK@ÆÔ¿êäÞבL¿ïó¾ýq?•¦í}XUNASNone?èFÞý©á?»1´Õ4O?‡%@ÒGo?zˆôU[âä?Ír0N'?ºÚ.GTí?æïħ?ÂP"À|åâ?Œ'óÖþ‰E?Žaaó}?ӐØLT9?ÁÄÜ	øô•?é>N¡<"ö?«?¬"Fn? F&HÖ(?£ì»\?Æõ;çóÕá?©*pJx›³?êß©¤æ ?š@¦B²H?"ts=¥­?qLy&IF?Áòغ–¿J?˜«œó¸–V?áP$ú¥?Â>Tj«?Ž²S°Édw?SÕËF´?Üj#mK¦?Âz}ib?Ú ß¯¹§½?ÇÑ!ºî?™Ãú¥©ñv?£w{ú†Ë4?â!pS,ÖU?Ç3}-Û¹?â«­ät?³¯žÈë\S?±Ã=üÁ°Z?_x2,'D?Ö7Ô·@¸F?²ªÅ~ä\m?ãþ38Þæ!?­½7›‡6i?£¼ú™O!?‰¨î¢?Ջú;½<Ù?¬£Á9ìkìMIXED4FGL J0654.0-4658?äp,·²Î
À3
#Ä*fÜÀ;ja©ÊÀ<Y­}|,¡@yåŸ+ª@ù7ªÉm?Ãr(üÎr>¿±€ð«NLê?íçAÃîä@ƒÃvŒÏ1?íVþ–¶¿êŽ|/%‡¿×Jä•@n…¿ìg«ud0+?½ÍË`¢=h¿âŽ9žÝ%`UNASNone?ï}bŒš¶-?'0?'O"?P³p{ºJ?JÞb-Gš?Žú[Ә?ëæå"?ïM92•m?ŽÌEtp˜®?e‰ÒïTã?r®IÍ©©?†Š<î?Š¢šÖÂ?îߧè¼Âi?/¡d[wµ?vQ¿—-yM?{.|DÀ›?žv"3Z?ŒFMÇRT?ïE±+[£?y‰«</?FÖµÇVrI?<ï³sõS¼?–•"(ì ?x²|©p¿—?îóæUIé?˜(HCq·?f]§-ŠÉ?_k&ó`à?ž·€~M_p?—½•´?îþããó7£?¢'uü^?r2mnx¼?…°ƒŸ­?›–蟾³? ¸èq÷r?í¼4sÐh?œ9ó'ê°?gB—>G?'"‡µ¤	?¯âó0·ùn?šnQ»;?í0Ì"ò?ž:­Œ%ùË?dâc{¿,ë?c,ýi˜º?µØƒAkð?Ø?üØÝAGN4FGL J0656.5+4218¿·¦äw6¸ç@2ÄÓ¿/UXÀ:û
ìQÍRÀ<~܏¸oH@ êÝïßÌ?ýÚy°Æ?ˑ<ÓÅåR?Ƙf?Ïú?üvÕIs™@€ž'&ޑ?痢–'R¿à'ƁY0ô¿³ðýmZ¿Ú7Ûu¼Æ¿æšaÙ¿Ï×æ'öÀUNASNone?ï¿ßne
v?jŸ@6£Ã{?Q¥	}lé>?AD'À;?{§N¢í?h^¡p߃a?ï5ãh	?—(@ɛUa?|ßgnUs?xЁ-V@O?˜aœî†ÝŠ?"/ða6?ïpa˜\"æ?yÉ1Ò×ô?d¼YËî–?`j'ð@»£?Ž¸uÈq,ð?wq'ت?íX7—Ï%?Š)'øî?ŠOµiEô?g×Åòª
?±ôPé¢Q–?‰ºÛàEb{?ï€sT­Î§?|1ï?2å?b6<S͚n?S;+0Î?‹U›¿˜ï–?yì3dl?íe#£Ñ´?­^{…)?Ž*r…³§›?'ÞÃa—‰D?¯Ÿ#zÔ?©»<½Öú?îëº*Þ¥è?ˆFî­Ælù?p-†ÆJY?hÂ%t›Ã?ž}Yþ'n?†"Égcó?蓼Jý?¢š·Éº²?œø¤?Z ð?…#J—Y̛?ÊúJÖµP?¢ÿRÐÅEhAGN4FGL J0657.4-4658?é‰}†'TÀ2'¶|(o‹À:ÈÈðŸ:À<›7W…"@Ý)ÆøÍ\?ýËj|uœd?Ì<>Y'?ß<Öàvø°@
¿Þd¤ÅG@Ia}žf]?éù¹à?Óë{#6æÇ¿Ø«€ÁF¿àå½^šÀ¿ïþ°_-âç¿è1ö½aÿUNASNone3FGL J0657.6-4701?îøº"?¡Ïô"ë×?£ÙÊ%òeµ?Lä–*?"­TvÌ;?‡V)äG@?êªH»'*^?º°šýqÛ:?º_"^;?µ¦n¿"bÐ?°N¡¿N×?¦áœKQll?éBå­:ؐ?¯Üz¯g™ê?½Ÿ›ÒP?¦f8»9P?¸IµŒCŽ®?£ëwÖ?éü…0DÛ?˜X¹î\º?»›Ù¥MVö?•àt?´üÛ…]?‰R>Z;‡V?ëñ1Ø.±?°Ábƒ<fâ?·=|›p¯!?­BÆ­†²ø?¢qéC©a´?•…G1?å,¸«é¹?ǁ—ž†')?Ì@+á|©–?źyX[‹Â?¿FBw§_?´Ú†«4´ƒ?ä—F®É­?¸‹¾&Ñ,?Êg8ïñÑ$?³ºcU=?Ã;®Óxɧ?¬r—0º†D?äg6£ˆ¹U?©ypðH¡?Èvu~(Ç?©
Ãaø?Åíü^ñä?Ÿy``ÛAGN4FGL J0658.7+2318¿à9Ò	Þ·A@'Ñ"D¿À:Ï-˜¿À<eÅööq@&=Kþ@غ@Ù$?¸5%¦­©¿'µÜïB?·/ù‰@ѾÎ]?îÝ)4­¿àø»Ó€E5¿çË¿m"¬¿äsšA	_¥¿ãbá@øÔ¿Ò&c«KžUNASNone3FGL J0658.8+2318?ïcÊL?«P†e–O?TA¸¦Ð?p*?uâ|?'Xë1Dy4?ª3˄Y]Ã?ì)Î?§™Üõâ?hÂùî"ÇÓ?rŒMô‡(?¢Šqšd¡?¦§hº(°M?ï½ó5ò?ˆœQ†¹Œ?jsUh	z7?a&âLý¾?š™Öðt?‡\8ÅVQj?ï"NÉ>Š?`o9)ßzä?Y€4¦ÏYé?8À¡•€Ì?‡¼G7"Î?_‰Áz€D?î¼maZc?d*ò¨ñª?aü)´iâ?RoçAô?£'¾"r7?œë«_>ÔÒ?ìÑVVÎÃÈ?¼îu(¡ú?w‡4…g?‹¤J&ޞÙ?¸"Ø;VG?¼‰ê–À?íÌü½?›£þ}æ?{ÈhœÉX?q|ìÞש?¯·2uKZ?š,k0	9
?îžQ"0}?­ò;¦/8?sØÚÿ?[Ë؛	Ç?£ŸË_TóN?~u$ߦJÚAGN4FGL J0700.2-5118¿éI×SRQÀ3‰æÿ}úÀ:ü`8NûçÀ< !¥l5³@—€Ã^äè@óû¶Å$?ÈW2ÁÉ8™?ºäù}º–?ð] ½é¨?õs˜Ôw¼?ïû¿ß(™ý¿àCòÖKҿҁ~ƒ=¸¿äÐeÁ•a¿ïÝUE¬²{?îíŽ]ü4™UNASNone?ï0ïÖˆt?'ÑÔy¡?X©>–Sj?R§ÝŽ?˜`3qq‡W?'T*t~Ê9?îþò9ÿç=?žÓÌËi-?'|¼ÇL¬j?ˆoï¹ý5w?–ãZcëæ,?˜-itŠ´?î^í6àÍò?™ùÓ»à]§?ŒT6ˆß)t?ŠK‰||8œ?¢üòOƒ?•Á"ÿE?í3'
¤È?'ø]¾.öÏ?—\NŽ?|ɘ[k?±'ÄDŽ^?Ž<Ü{Ht?îµJî†?h÷Ê®7×?el‰Îoï?bR:û¬?£Tˆ€]+¬?œ®…kd?ìú¤;^$ù?µ®*l©æ?›É5e'ý?¦.ñæ#ðQ?±8Êèññ?°¦="T?í«<sü|?ž*>©O˜?',èÒx§?‹Ì
ãI?¬µÊÝÌ]î?š¢@")?çÚL^ñ?©ú,.Ãà?ªdž¦xï
?˜o׸À?Éý§ð
]z?§59ۉwAGN4FGL J0700.4-4308¿ÞVœ€À0¤a¶Ô=À:ž;¼n°¸À<AäMòÒ@ý¦kd@8—Ü*7â?ÄÆFuÛ#}?™|cÓ¹ü?ÐԁLá@©zJP?×,B®{S¿åV«€'¿îÆ!·à¬¿¢	_$RÅ ¿ïÿÿ" 5•?ïó@oܲUNASNone?ï§dˆô8?Žõ¿ÙK¹?áp×è?^H'^XBê?³½"ì2?Žâx´{?ï½óå"B‰?o£×V,Î?Y\/â		À?pÍ"8¶>9?z¯Lëœð?zG²duYK?íüÉ=ºå^? xd
ƒ¡?w†ŠbÎt?{=^ÂÇ}?­BšÎ/Êß? G™3Ҝ?ïÄr

¯–?eItš[?S[½¨gt?B¥·ùü;?xð7I¾ ?cD'Ãw°?ï‡\eJ?ρMú?oÚI	x'?o´|#0–?†B-`±&Æ?‰Ä`MºÌY?ïH¢4Œ"f?EœR—¸ª?n>ÆE¾`?((UC/S?"#àžª"W?—RDø*ê'?íh&ՁÒ(?¢ôäJ¾?ÑÌ@7?ÓctÛ}v?²Á¬'ðˆ?¢Hùd¢š^?ï*Û\ê?ˆ;€±+¶±?v·5î?pá@ºîȇ?•$f¼¢ˆ+?†(`D®ó­AGN4FGL J0700.6+3558?鍛'Ž@1Cð#éêÀ:¾í¥Šh¤À<…˜f"³@þBƒ2O?ÿ'
;Qå¦?ËB%ŠÌ?Ø#ïÞʦ,@
9'N"¢Â?ýNÀ'"ß?ì'JSá)¿Ðè=µ¿ÜÞÝÛèɃ¿å¬•õ *­¿í`Ÿb0vÀ¿ïþ~á•›UNASNone3FGL J0700.6+3557?è䑷DqÁ?·èt÷brr?«?*¹ò=?ž9]yÚQ?Ũ)X­¯ë?´í±Z%q?é8r¾Ÿž¨?Á´"؃J‰?¼`$1Qu'?´b±'79?¹ÜEÙ±•A?¶ì´ƒ0ÊÄ?ê¼|jFC?¨û ªìé}?±@8šÊGí?('X·æ²?¸Ûä¡yx?¡Â!5iJ?ê%:€É,ô?"Ò.pÌn?¶RÆg™G?
ØÀ,v?¸"1)=?Š*k¹a‹?å%ÝñH"?¾'³/9Jò?³2ږæ–4?¥éx%Áàª?Ñ.ý¾Ü
?»Ò>!‰ù¥?ãQZ[sÌ´?džºé9XÖ?̂vr"1X?ÄÀÄ£*	?Æ8 "4]U?¼¢-ð[п?ç¶8csÂÅ?±
:םŒ?º''ÙlK
?¤^hchE"?Ä]zÏe?ª}zùÁ.?ä°Ú8£¾?¥"}le¤?Ây¶	Íð? ²úЬ…y?ÊÃxgg9Â?¡$m†|mAGN4FGL J0700.8+1551?Ð<Ó­3 á@"^ËtÝønÀ:ÕZ±&~À<u˕•(@›Ãl{Ô7?û6KÄúp?ÓoI#Šs·?ܪù=n˜@Õe!ÂÈg?ýiÀÆY@8?ïøc‰<TD¿Õ×u1ÛD_¿£âï#
÷¿Ümz÷÷ž¿èƒÜ=®l¿ïÿËÝcßUNASNone?ìÄ`¹ö~?¯6ŒÈ¿'?Uô§|ô,?…£]S{™?»ohBV?­2C§¨-º?âÌù|ûu¤?Ś³Õ¯õQ?§ó<"2Ä?¢¤e¤š_¯?×g¥uðÇÿ?ÄX¥Lo:?íZÝ#æ? Pª=Ýà?"Áøf©Ü?‹9®y.þ?²FŸ*5Z?›–iúI?é~ñ°0+?•ÅŠ®bø?ªêâzr²±?…ÔÃwt¼Ò?ÃIƒRk˜æ?'î+ћçÈ?ènJ¶\ž?»Š0³!?£t~žiؤ?œXÄä·?Êñ',C"?¹´±¼¿Ó.?Ô4÷í?Å7è=…`k?´&§WÊ?´ØLþ»{N?ãel&Г?Å=ì6kï4?éîq–VO?©‹‡–¹t¾? aáßh?'î›°sp}?Ä@¡-À5B?¦éÔå2ê?ãÒùçY\?§W•F±fÖ?±Èœ{5X?˜âî |ÏÄ?Óçåaþð?¦{/Jk?0MIXED4FGL J0701.3-0403¿ã셾½P?ÕÏæݚ$"À9dYbqå À;BöÜjς@aR½è@Rr†/YŠ?Æ-¡º$?Ͳt†åŒâ@%ÏÅ¥'?ûPü#ý`>?îèŒEô?Ð)ú¥M,¿ênar
ßW¿è"»ìª¸¦¿ïý ‡_r¿àÕ,ß?–UNASNone?ã#yƒñÞ÷?À­44˜—?˜«.Döyû?Ý¼þª?Ø.ZD?Àoj/d?ÓpOC	??ʄw­îÕ?¾.e‡Ýô+?µ>*˜f?â'­¡î?É¢:Á¶²ô?â3t¿°Ö?²¤<˜F+?°0 ¸›E?š ûyOÑ?׌îTJÉÂ?±ü–`?ۛ©òµÈ,?§øÉ
7 Ý?Ǖ¹ÇȒ?Ÿ"lŠÍ
ü?ؙͱy4I?ªþÓ¼~Ð?Ð4ÅÚjD?½>:ôÙÂe?¨œc,í?£ Lq_Î#?ælœÌ\˜?¿ž"‰©%?¾¸Vô›¼?Ào=g6?ÂXa[ö²
?ÀÎge®ŸT?ç'Üʂ?Ɛ3ùE•z?Ô
­ÊöUT?²Œ–R.¤m?·`4müÐ?Ÿ€¥®…!?ãÝ Q?´
‡ßC-8?ʇ üB
õ?¤¼%ü,?ÐÂ՛0%??°E
®×/?àü¬óWiã?³åYd	ÓMIXED4FGL J0701.5-2842?Ü¢;6@YÀ%GOøe×ËÀ:ûІ•°×À<CgUy¯@lþáòο@Y™~Á¦ÿ?É<Õ"oß¿›'Z¹gž?Òo_Éî@×~I1!`?ïݬþüõ?£`,¡¯ÎË¿ê§ýuDØ¿âTÁ"tŸ¿Ò‰À¾Kª£¿âª†7"ëUNASNone?ìæÊa?³a"‡í'i?c‰Y|"dy?\"Ä!Ÿc?¿4…$¹ë?³/ð.aùU?ìøç:•?¶bô²ÖÖ?bœÓ¦Sèë?jã®<s5È?º™6ÐÕ?¶ïöˆ?î>¶&ˤa?•td²°aŸ?sï	Ú<«'?n»$ÆL1?©–¼Tæ~}?"•¿…ã?ïj©õí?ii§¸êb?M·[~rÍ?6$Míþ@4?ŽIß¿e'™?h²Kfº¯ù?è°¬}|?À.ùß÷Ä??s
Õ†Ž?l…dIPäô?Îìæ¦EW+?À);ÒWë?鏖[ª(f?ÃɘçåNp?hº\«$M?zñH´§•?É^½ m™ó?Ñ(·÷9?ë£ñP²Š?¦ÿ*U·?ƒM fI?xG.úÖ«·?À;j{ì,?¥#ÉZgÛ?îfœojy¤?ˆøҞ
–?eéiò'F?W3°ûż˜?¨DÚwÃÅ?ˆSyvNëêAGN4FGL J0704.3-4829?Ô orZÀ1ô$¢v·íÀ:º¶â¼yÀ<V "oeé@ ]¾!8_?ÿoÕ`EK?Ìvô©	Ï?¶vS€ÕS?ìki¥¶Ž@ëuró½|¿ïñ±ôr{?ï÷á]¨|¶¿çi2(q8R¿Ò±K¼ìÚß¿åžbP2¿ådi×4.ÜUNASNone3FGL J0704.3-4828?ïۗÈ߃?a)¤Àq{??0p.ZÊóT? '^q¸!t?q-Ä|?`£ÎðICã?ïãõ#iLÜ?oÆDõ^ے?5¨S¾­æv?B¦–u­Õ?iUÒ$9˜?lø#iì5?ï˜^3ù?r#"Ñ/˜?T^``%r?PÅɘMàÒ?‡\¦ì_܁?qoê+&ÿ.?ïj³;šú‡?k¬ˆÒåâ?b¥>{ÂR?DM$G¯ë÷?TðÔ0FÙ?kHë~+?ﻑœRº?qÅ͓ÁõK?@0Bt̛¹?4Àx•Ö@'?€"µOöÂ?q9¼åÓÚ?ï¬Jø»æ?…ÅήãÔ?KŽKã;Q?\‰çÇ
hô?ƒ4]Ô5³?"R0jo?ï/Hnó?†Ð¿à®–?]N.™•ò¬?P²3°á?˜BX³Vv?†ª¡FÂ?îŒyTC'ì?…­/èB/?sÚ嘁>?aS§¶2?¤½½ ?…xAøKj\AGN4FGL J0705.8-0004?á$÷ä±#@	\[cÓåÀ:"Ö¼À;¾7¹ª±@¥pŠí@¹÷<âß^?ÊàÓnu)?ÕYâµí7@ñžBuÆ?ü¹¼yÃep?²Áýäê%?ï\ÂMÂÖ¿âQ%!!¸·¿éè¢ì(²§¿ïì7Ì'ã?îi,êCÖUNASNone3FGL J0705.7-0006?áqs¥
³Z?Âþ±~ñ*X?¤73Ô	Ü?œBûʈœ?ږ2;¼n±?ÂÒòBt'?Ú¸h7ˆÅ?ÊØ
)«—j?ÞñMÆÅ?»€é@î)5?Ûx!"‹y?ÈR¨.ùn?âqG(f.;?±ŒÈ<ÿ–¢?¶$»•'¯ã?¬ÞhÊ}?ՔBɍs?°.[Nñ"Ü?äÀPƒŒM<?¨8"î'?ÄÒG¦îÒí?¢\''Ð?È,vJßø#? $
¤/?×`A€ EÓ?Á'«å\ÌÆ?²š#ª,£r?¨+Èx™?áüšÊ"ƒø?Â_VO "Î?ÈñýL¶*ä?Äf—=¿›?Ï;é>ŒF?ÇVœná	?áô†]/c£?ÊþŸã_¶I?הø7è,W?±‹‰®?ÀHUÁ¨?£žðT=#_?à#}N›´?±Ø0KÂä%?Ö©?è*ÿ¼?®©¡Z bö?ҋ½†F?³0»Îf™¬?Ö˼ZÓyÿ?¯WŸ€É¥MIXED4FGL J0708.6+1747¿äÎy…eý@'k͚R&>À:íÚü:x¢À<c;8»2@ ‹34à²]?þ{®—WŸú?Ð6[œ2ü?¶2ðÞ¤æ?ꖉ1+?ÿB¥Áðü¿îÉÔž›·?ïý¨6ëN˜¿å-ë?ÿtj¿àȖg"N¿×R[ø#h¿åû®Í…/UNASNone3FGL J0708.7+1747?ïiØ;Ébh?…v&ÊZ†Ó?FR"Fîaé?5ŠØSá"o?'gz|a¿?…-V™h?îÞûi~"ü?¥#ÈDóg%?eÞÊ8iô?l]Š. ‡	? ²hyde?¤Vt­†Hu?ïý­"!?ˆO¹ð‰çá?eö9¾v̈́?[}ø76ˆŠ?šÏø *?‡"ãÒ_D?î¶0îV× ?{ÿžg¨ëz?u»ùÿ¬'M?[¥,FÈLô?¡åqÚôéÞ?{v)2Äo{?îøV†??›!vŒ6R?[ù^Y‰U?Qúöå$áz?¥GúÐÍ)Â?šÇR(Z«â?í<Ç~?¹B#ûð—P?zÿ3'¦ÕÈ?‹s ¢Ñ•x?µßZá"|v?¸ƒëßñô?íÕp¹•QO?ÓþÙàÀ?r]ºàsã?iNç´?°.žŠ*w?œÔg¡÷M?ì¯búSÌ?• ;|áZ¬?"‹¦rã$è?uW	í¬j?·õõ?–ѵâAGN4FGL J0709.1-1034c¿Ñjfõœ=¨¿íKÒ»úÀ9!ÌzdJÀ;1œ_F·t@üx±—'-@ÁåGíÕ? y‡«ZŒ?ÓÊ89W@¦ÜG©ã?þ0n&nª¿É¢ãj_D¿ÞÒý¾\G¿èQÒ?ÓT¦¿é°‡ÿ=¿ëoc/zA¿ïý…1,ȶUNASNone$?ÑuåK?ÀÇõL¼?ÍGòÕÀf?¾æÝã(6‰?ßæ!¬N?Âá3Ü3{?Á‡Z@­?·Ø®ÑÓáƒ?Éõ3ÐŽ?¹<ðYƒyÔ?å=ÝBú?¿ÃCæM–%?عŸSAñg?±¯YÞ_ö?ÄÜ×[ñî?§¢*6?Ý>rA¢?±;BAß?È·yh÷E?™õH´'N?Õøcòv]2?£ÔÌÈ—ã?Ý«ßZ »j?£¢±~?¼U®ä?²åé˜#g?Æqõrª¹Ê?¹ø¢Ü–÷Ü?æØâMx¿ë?À\¦«ó/Ú?¤+ÆÎÎ2<?¦rþ«:WŸ?Ë+œæÖ
?Á§ãM0¤&?çú8«Ë¨é?ÁžÐÒ¸@›?ÉçÆ~Ê?¬3bJPoÕ?ÆQúË°?­¶š9a?ãñ»tz¦?´;Ê5RN?©Ê£ÙŒÄa?†'Rê®k*?Ü̸@‰ï?¯:éTÕµÎ?ßùóD
~¡?®DnU.kßOTHER4FGL J0712.0-6431?Þ Ì‰!ÓÀ6*¦óõ/ÂÀ;'24/²uÀ=ï4Ö¡b@§!,JŒ?ý8ø¤ÁëÈ?ÑUØInß?çï~U@Jâ|az?ùÜ÷&èw"¿îªi?ߓú?Ó߁w^¿È*è7¿ãÆ}'s¿ïÿ¤Á	?¨~¡½÷¿6UNASNone3FGL J0712.2-6436?æ3…€²íÔ?ÂíèX÷ñq?ʳ%±ÀVó?À6êhÐ4G?¸ýˆ—ÃÊ}?±+ƒ¦
&v?àä¨Ò'Õn?ÉqÛz¹×?×	ë£tX?ÇyÍÿÛJ?¼³
Ùͼ6?°Îƒc:¨?ᶼPd?¶ú&EÓ¸"?Ô*¥<‡g?´FW³]IŽ?êÏÄEa+?ª›žðZ@t?çB1I4b™?¦~yÁW»¸?É<a‡Pä?¤|:°wy?³u²¦qHŒ?'¦)?ágڇþð?ÄÚ¤"aØ?Ӓe>.u?¤Su·«í?Ã;Ëc§U€?·'‡—
£,?Ó¬ŒÑùÌ?ɨ<œi?ààrësŹ?Í>TN‹Ô4?Å%õ:²·?¼u4h#J?ؾP^X?¸[LÇ­?Û=ž?¹®Îz5s?È	µ ÝD?°…(?ßëç¨"üã?± `¨a]"?ÕQÐLÅÅ?²_R—ܽ÷?ń¯ z°?¥?R¾CMIXED4FGL J0712.8-5637¿íöÔBëj¥À3"µþT.UÀ:¢P0™û¿À<bg.'Å@ôê†ñ÷)@"dUêî ?ËHhbj?Öq"'›@x—Ü*7â?ÿ5Œu?æâ"Ÿg9¿Â'N¹Ìiû¿èϕÔèû¿ëf YžØ¿Û<-'ÅË¿ïþæZ<ŒxUNASNone?ï1é²
Õ?š¡Þ WŠ?rRr{æø?s'qZ¡'T?—…&3à"?–û'§YÊ?îéàSV-?›Ä IWˆ?‡Åé?Œ
É^bžÌ?–üokŒ"Í?"'Š¨\w?îTª¯Ê?—Ë¡2ýô±?'w2W[?Šxä]Ü*î?¥²•Ç5?'´Öey?íjÎ5é­?‹-.S¨Þ+?˜؉±~š?ERãb›?­F°Yøº~?ƒ´çy[––?ííÙ³ÿ»%?¦>/5ƒ·³?…MŒà)Ÿ+?'+âÉát?«Ï‡þß?£‡ˆDé†D?ìWMuÃjg?·V+Y'Ï¿?§zcZƒ´I?¯(
÷j?±ˆb¦Z Ÿ?­îß6Õ×?쟤U_Wÿ?¢zÍKƒÔ9?¡?ä¨}æ?"ÿ—^ݯ>?²|½b±?œ½%a?èbsØiãô?¤Ô&ÍéJ?±,ù–ná?ˆ‡úF§?Åß³ÓÆTý?ŸA;¥qAGN4FGL J0713.5-2555?ﱶmÀ Â	$lÀ:`öqÀ;ôó±³l@"®R
hô@éu½~â?ÂC| 7?•g'ߐô¯?ÖÑá^ª/i?ý¼&1$4?ïa‹€|<<¿Þà¾FL@¿è´÷Ãñ[ø¿èû9Ç¡ë¿Ð±©ûçl‹¿æD˜5kUNASNone?èï|x‡·U?Âyèlnî?t¾KŒEs?i=¹	ӓ½?˜"—¡>?ÂfKXÃæt?è<öž¾"?¾d(.Ùm€?s	"6/X?våúæ#¬¡?ÎsÚô"÷T?½ô0¨Ð?ìV"Î2ö? ÕÊÍQ?†ª±–{Ý?wkqšm?ºv	¶Pù1?ŸéØÑ[àx?îF²š­¦þ?ƒ^»Úß?r\™Íظ?Z7˜lxÇ8?©IC"™?'•ÐØ?æA=ü©£?Á÷‹¬	øk?'þJÔ%ºÜ?rfÞn?Ò呯•Yn?Áó*"–9,?à|:Iì¡î?ÅäÃßO?z)*ÆP%?ˆ`™¤ª?ޟ6Ç<j?Å[k¡
×.?çA­¤ã?°gÞzä?–Ô à¦…?"›	¶V ›?ÐcÏwñ?¯mIÄð	"?êöóþé? Mʙ?Šƒ²ÿ%¢l?zҝÇ}¹Þ?Â{øo¤
ø?žµlfftAGN4FGL J0713.8-4820c¿Âé@µ#tÀ0q+àŠðÀ:Ä©°ãÀ<G#çÆM@«<Û}"«@âÑk—þ?ÉâxÉhi?™OSǟ³±?Ñ&±dç`L?ý¨Tßd¿ÖX‹ýy½Ü¿ãCÿ~zÚ<¿ékEÞ±{¹¿Ûý¥|üªá¿êöÁBU&¿ïþ:bÒ]0UNASNone ?ï{Nð¨õ?Žºd#'?d|0õ
Å?WùaÃÒó?Œ*ä½ÖÑ
?€ۉÜØ?ï¬1µ•ß·?à;"­ª?Z…NŠYç#?d3´Å¿qU?¢è¼Þ=q?•5äïÕz?ï8P‹Þ›?…ô·y3?q—ɑÌv?okgW'.B?".TßÒÏ?'kæ²÷x?ïg¨–ô?u´¢ §?r¾;V¢??RÅZ¬º®Ë?šŽä?øA?sí¨Ö ¥š?îÑá‹Q¥?"ëh$sÖ%?sý=±Pv?g%¨»]0? bGïi)?"©ñϒYF?ïÚ³iï?ŸL^gc?qÍïnÉ?€¸6" ®?›?v$®çÞ?A]ñ·c?îšÐ@Ó7~?'œViAƒ?{¿š#sæ?vSP£sD–?¢Û­VBŠ?×SY0'[?í[( X?'6á8¨?ˆh7»œèr?péкŸ?²¸MÑÔz?øX뤩AGN4FGL J0715.7-1128?î˜I,;>½?´ÿ¾'ÜÈÀ9¼÷~0ˆÀ;`Πâc7@o!c'Å@¢Ž…i`í?Î7^¦~"j?Ú°km6d@@º°k?ꏳ`Xôþ¿Ü*«Ú佄¿¹ž+࿯¿èðCÊZ+Æ¿êN›n…êLžsóí£¿ç+ áCUNASNone?áfZ°ƒI?Ì©˜íC²)?¦ü`ᇽü?¯5^ËVD?Û§.‹?ËPpÎÒ¿?ÈÍ*ë'&?ÅI'ú?ÄG…×=¤?º~àÆ(î·?äºÓÎÒ>.?ŦØÇVì?ݽSØT¸?²H¡êÃO?³íøÛ7b‡?œûÇ ¸Ó¹?ÝG.ªYÒ§?±ÊgÁ­?Å ®m³"?š"¨É^¹?Ù	"ù,ãI?ª™Ñp3?ÜfÏùZ¨?¨HE	?ÑÂú·§Ý»?ɪz@˜?±iMùís4?²ìÆüÎÿ?äñXä·hü?ÉëedïÔö?­1°–Õ&à?µTÕè{ë8?É*?Ã8¶j_Å8?çëÞ6ðÿ?ą6oA›?Í܇¢B¬ð?®ÛÃQ!Pu?¼9z*èŒ?¤W!aêú·?å®Ó‰÷²?±Ë‡û:3?¨¨Ò×Û¢?‰‹J­jŠ?ÝQžü¸€?³ÑyFŠJi?ߙUëÒL?³"¤3ÈÒMIXED4FGL J0716.0-0826¿ïQ'bñðP?ù<¼~ ïÏÀ:$OTÑélÀ;¬ÓW*‰A@ç|\@?"Àh¡?Ð(Zý|˜?Ô)ù"Á ?ùb.þñG?ñrZ5*¯+?´Äúâ‰Í¿Óãº¥¿èq'>3Av¿é¢á ÁÁ¿ïøìˆ3@?ïÂpóˆ"yUNASNone?åCæÖ¹5?Æ[Oû?žñ¼ì&A?¦
£lzÏ?ӊ²cȄò?Å>…¹_T?Ú&¬žüQl?Ð%+ÏÊ?³³ßBó'?±sÿå<«
?àv-Îð=•?πh+s²e?㋣Y-e5?±¯ô¿æý~?°®l7×Iã?™Ö—…?Ô½@TP\?±WÒüq?àI^šâf^?­½U}¢?Á²¸I›¢?Ÿ%¾%v#?֓æÂer?©]HƒÈ1?ámûøÎ?Ç«×òù9ñ?¥Â>ZW?¤Ím6gE?ÛXª'?Çx)>_-¯?ȶ4DçL?ÈXh¥Žx?ÀerlüO?Áӛ#˜œ«?åÒ S‡?Ìf
vÇBÛ?ÚŸ¬`Ï+?²eS<6=ß?¼Ý÷›Ç5"?¢ù,eßcð?Þ®âl­cŒ?²Ül1×h‡?É
k~åI'?§¤yûÒEs?ËàíÿUà?°iŠ¥ÑY{?âÄi qhè?²"AƒMIXED4FGL J0718.8-5004¿êï{¯½Œ,À0Z\å´$_À:͇
JܝÀ<…f?Ð@³â@0Ö­3ª?Ëq}Ü#×Ì?Ú~FïƒÜ@¬>/æx@ ¸=s¨ï?ï›ÞÒê¿ÒOZ±&~¿ÜŽèÑQ­¿äÞ!ž`RÑ¿éO"¡2O¿ðUNASNone3FGL J0718.9-5004?ëŸi†û?°£ÖoŸz?­²GE¦â´?¢"ð634?´+"ˆ†Âj?¥îøH`ô?í_­*"ÆÝ?²	6šÒÆå?£Qú®éTE?¥!&x16{?¦³2°¢è?¨4Ê~g.Ð?êЇæ?ªè1V_S?µlì/¥?¢\M!µ¡?´ÒH³¨-?¡
;›*?é¨Q@w?•×X
õØ?²a,'¬þ?‹¶šA›g
?À./'àĦ?é˜@?çÃCj?º´ø"nu?¹²'š3†?­²Øà³2?ĺáè½Ä?´
Ÿ;%7K?èÖÊÖ8Âz?ÂJ³ãîž?½¾" šœ?¼IŽØÂÇ?»‹-ŸÜ?¶'ï1äo$?çð[GNs?´¦Íãù?ÃÃ	êåf¢?¯©ŸUƒ/Ä?¿ŠiTFB?¦9ïâg?âQ}¢±ßû?¦	M®Ý?Á#"ê`¤? '
ïbì?ÒËBEl=7?¢'âQ`ž:AGN4FGL J0722.4-2650?³\Üp¸À¬	Þ¦%À:ƒsñidHÀ<D)ÿ®@\ó4ëo$?ÿ:¤þQª?Ð=;"G?á%K~ƒ"ž@aL¾´?þšBѶÁs¿ëqA@'m¿Ú‹2äôQ¿Ï4`¯Ã'¿åËDÂ&ք¿ïý¨¢K?¦«Qý΢eUNASNone3FGL J0722.2-2648?â±æQ$­+?ÀRke\XÏ?³$ÑÜÜ-?¦÷ð½Çë?ÕÖê)vh_?¿–òº?ÝøŽ`oE?ÄÜÉÔ
͍?¯¬€Ú?¨¬…Ä‹(?ß'\ui?ÃX£Ozç}?åK"eI¨7?±Ñ;™Ï˜†?¼ÿšÜ|?¤;¶-†Èr?ÌQá`Ïðæ?­JÜG>-?èp¨Ì½]n? %F¿	É?²j'Ýø?$"¢D@ª?Å9'"åh¶?™ånl4Õ¡?Öóçì–tT?¾£´Ì65,?»çÅn?°.×H,½Ä?á%I,¼?ÀQ?˜qP?ÊÄý†º*?Ã	`Yœ?µ»\Z?·¼nL¥$[?æÀ­Îɕú?ÄÐÑýkÙ ?ßj50–ÿ?µ€â¦nb`?ÄD¡3…­B?­Œ-©¿(5?ÖÖE/ù±¡?µ ˆ¹1u?àìÒâ?­0OÇ:¢?½4S'€#?¢Âà/˜-?ÖÙUÊjz{?«MÃuhÀfMIXED4FGL J0722.7-2309c¿ÆëBS]öÀ:og—À9šñÎäÕÀ;LzÜ?0—@Cÿ‰7¢@y͛ÿ¥g?Ê»y'¾?ÓE‡~d	@	êºp©¶?üXùÁL'?Uª×¿å3éèwM¿èՉÕwõ¿ì;C½Äò
¿ð?ðUNASNone ?çä ZlÍ?Â9'·–ôh?«¸g´{?­ëøÈ9{]?Ɂ›'ý-?¾ë	M܁Ì?à"ÒϊA?Çñ;'?¬$xyF9Œ?©´7 Bd°?Ü5ËRhŒ?ÆW<î¯ù?ãùÜàk:6?³}·ž î¶?²}òøDS?žO²HP̂?ÓlɀÖÃà?±^Ú~È$?ÜQp.ªý?¬ Ç½7Ý?ÃZ0sÌf²?ž9)âêí?Úw—nϟ?©õÏnw…?á®J€¬¹?ÇfFUé…?¸¾º*"ÆO?¶z‰é5SÃ?×Äôà«ë›?Žgæ){`?ÆÅ}Á)‰?¤9t"¦?º×Ë,Â?ºè‹³ìšâ?æ󾍼8!?Å^ßê
ö(?Ù=h…j?´é}7DW ?»X½9?£y[)ª?à
ɤ›¢«?µ?¦©0g?"ñÍ?ìÞ?¢¡´{_VY?Îbãm*ÙP?¯)N?ï}S?ãÂJ°ÛÞ?°I$»Òý´MIXED4FGL J0723.1-3048?ØY=iÔRÀp®SeâÀ:¬ä_‰PÀ<<v`¯m@@ÅIìˆ)@NŽ£œQÛ?À÷5Á'쯿˜šŸ˜·?Ü´O'…€?÷Q•"&h?î"gñ€á<¿ç[}Õ¿å÷ù1~'¿çŒþ«—¿Ú¡ûÁVÍ¿³+ooyŠ…UNASNone?íO¦ˆh^?®I•²D»e?e
0RQµ@?\Pwéÿä?´Ú~zCj?­±I–å˜?æ%$ÛeŽ?À^atº3?zÀ¸)Å%Ú?~Ïïâëþ?ÓJ´íe§,?À'~>tYï?í—Z£u̜?˜Ö~Ù";V?y°pü76?n*.úÍ]?±ª*žT¸k?˜4M]­ƒ?í@µè.Òü?ŒL¹‹	Zˆ?€¯aƳG?d¹'Oø|-?³äd†Žæ<?‹ëu<CÝ?è¼6GöÊÞ?º'L¾þ
»?z}aýc?ma	§¿'?Ì;;ÏRÒÐ?º& ¹Ú'ï?ÙÙWŸ¤¯?ÄP•Gª?ÉÚÖ!k?ŽU¯qã–?âÌ,Ä·³?ÄAäð|w?ê‹ý©•?¨çOJ¬Q?ˆ-0ßÕÔ?wðD+ï>?ÆjýcCO?¨6ô
Ôh?ç­	R'%?¦VD-¢?—D]åÔÔ°?‡nÝàϝ?ÎcP2–?¦x=#c:MIXED4FGL J0724.8+3016?½æÍK@3öuy(àÊÀ;±™]3·½À<½`µL}‡@#nxY$È?ùÝ5µÄr‹?Ƕ÷xr¥¿¨ócå$?âEy¡¬'@šŽË·¿ïÿDÿ8"×?ïÿï0l¯¿æôpŸû2'¿Ñüf£".~¿ê•ïUÑ?áºæ ³iNUNASNone?﫦S«?‹3+mÅiý?BsY]Ì?;äú
š4É?"òçŽ#*?ŠãÖEõÂ4?x2ZŠ?"ëšEД?ZàPð¯ì?|
ÿµÀáC?…øáÕQér?'Žf²'	M?îwÑx¶¨§?™àðæʉX?pH¬Â£¤?y†½%'D;?¦yæM5!?™òº_F?ï$©<FN»?ŠuÑ'_´?h:&X—y?Y%³3ðZ?˜c"ª±«?ŠLë2ýÿ?ïl¨b	_z?– {)ÿÉH?T9'[C€?Rþ†÷·!a?''[œZƒ?•ä,¦Àã?îø'âaÎ@?§µ¹B¨Ý_?g!RŠºLM?w.sÚe
J?žy\—˜~?¦ÉIù\ó'?íì=qêAì?œÒ<?¤ÅB?q°åûî ?výY-×øO?¯$Äñ?œ8ðä
™?í
™S%½?§"žhAz!?'"0íìS¼?¹]=w¡¤?µX¯G'ß?§Í
èÄؕAGN4FGL J0725.3-2550c?ã øBÇOàÀ†¤û¨'À9Íí'?2EÀ;c¡®;N@-8œ(À@Åôÿý²?æhàÿ‰¸{?äužö$à@
-«Þ7@È{"ZÃ?_î}!¿á¼üJÈü¿èÛrLM¶l¿ïün{Þ¿èÁÞ\AIv?хõB6Ü5UNASNone ?åíõfsý?ÌϺ#8$›?°$[¬ˆ†?°üð|M…#?Ñå
*µá#?Ê9úŠþ©Ç?ãju'sý ?Èí
TQeù?¥bA×zuž?§©sèkJ?Ö~Ì¢
9,?Æ{¬òo|B?ä¤2Wý(E?³TêJ@~?¶=À‹#t?¤çüO² ?Ñ(Y«ìØ?±,nsh<?äXÑRm‹?¯{N?µáûwÎüO?£üË=ç¨W?ÑÕÞ|UC²?«_Ý^‹Ó?ÞÙhZÌ6?Ì"-Q¥m?º³ë»‹˜?¸öw£9Ý?ڟ*ªEä?ËYê÷Úí?Ñqâgá?ÈÕ¤=GÅM?¼¦‹<-Å?¿ƒ»vc3¬?ãÛu§L	Ä?ÉYDKÖº"?Ü?¥I í?µÜÐ,i¾?À›±2"Î?©tgáÉ5?Û¼ŒÝ7lî?µÙ°{ïuÕ?Óøòleü+?·¿êÉ!b?ºÚM˲<ö?º»± »:Ã?â¨=à*«?½m"Æ	ÓØMIXED4FGL J0725.6-5008¿Ýô•Âä/"À.À'ÏR¹
À;/ìVÕÐÀ<"ՐÀ­@ ÃÉñ%F¶?ÞW> YQ?Þ%œSÞ$?ï‡ÁàŠ™Ì?ýC·zU0´@-'U°5½?éQS¿Å¨@?áµVÄ1ó˜¿ëh"ÞÒ2è¿Â2ÏJ«tã¿ÍGöµÿV¿ðUNASNone3FGL J0725.4-5007?îúu®q±¸?–‡Y{7?d¯¼¶Ì$Ç?`†Up%&2?žR–мq?•—o*¬½=?îú7Ǫf?² %	?rgC¤?‡)¢ˆ"?œ1mF™Q?±´×&†Á?ît«gf/y?–þŒy9?"¥V>º ±?…"£Å¡È-?£‹óùî`I?"¯V°•þg?ëŒÃ'LÒ?ª҂-<?zlrƒ¢?yÊ)wÿ0C?Àù'íFٝ?ª'"NÉ32?íû"Æé*s?¨ž H=º?|h¤Üù`?w"GÇS4?¬¹®üœ)?§¾ÏÇɚÎ?íÏÆßwî?»BŽV*À.?‰OôÍ€,?¤EÒütÈ?¬¯"Ø"¬?¸$®¯,2K?íwú`ar>?¡$d3»?‰|­'À?ˆ¿éP?±©ü?ž¦ê
»°?è´Ñ¹[M?¼ÞáP¬.¶?xjûÃz©—?ƒF¥P½úÐ?Ìia«Ê&]?¼÷y*°¥AGN4FGL J0725.7-0549¿á`ґô@¼ŒÖ<¸À:$ÕϪ͟À<'¤ýzê'@ ·E¼wÀ?ü.;—…Ã#?Äãâ'§ä¶?Ã"?Zˆâ'@üäŒØ@s	¶Z?æÝÿŸ²ãB?í€FacGM?Öå±àHþ¿ÛOȶ«¿ÜìØ:¿¯¿äJè0-UNASNone3FGL J0725.7-0550?î–1»õö"?•q7E~žÈ?bÎ!؍5?X	è4%?¥s\áD?"ìžãÖ4È?ì«"ä¬è?µÂÌÇ- ?l´f
úä=?v‹Üþ¯Y0?¹ÁGÞeü^?´ü·
1ç?îFháëÃ?•9á÷L?rÚ®cŠ{à?lg)™$So?©C©»wP?"ë…l‡€?îüҒÎ=?ˆQGÂ͟¥?xÃó@?h¤ïyz3[?ª2$€ª?†=ôØ.ª¸?ì҈:CI?¨o]*ßné?|۝þ‹¿D?rˆü£Š\?·žN£?§ÊŒÁnö?çݕC7|?ż{{¡a?"kíìö?"ÖøP€˜?Ïw"Cϖ3?ÄùåÕ'?ë_ÍùŒÁ?¦íj¤ñ?"N¯Ã®_?yœvnh¿?Á;à‡Oü(?¥¾|
Rà?ì²Þ¨Ü? UXlÀ­?Œ×Çß·´?~¤aüÐÇÂ?»¿p),?žËe¶Á‡DAGN4FGL J0731.0+6607?å°¢Î@<ž"šVWûÀ;	µólÀ<°5ŽWF8@ß\>oQr@N˜™¿YG?Ï^ç–ýˆ?Ë
ïWúh?ûѽ¥è@$ÃÆ=ç?Õâø]I\??ì'©
Oå¿ß§ñ¶'!%¿àt`YÜë(¿ïÂXúìñ?ë6ElÛNUNASNone?ïIÐúÀZ?‡%ý¶;Ë?{/{l¬¬i?pjA"¦l?ô˜Fûk?'À'L… ?î÷ùÓ/b?š•gØAÐ#?‡3xóô¾_?‹˜À5?‹?•g	 %"ƒ?ŽkÅ×"*?î•Nø¥\Š?'ÍÄkÑ?u0'iàŸ?…¾®¥:#Í?ž›ˆ¢Ÿ~j?Š!1H\?î¨"GõÚZ?'R­uéA?—:L쒛ì?z€)^ß»'?"Áj!´Ü?sr›é?îO¿wú?žO¡AÈf%?'b`X–€F?…ã•U&Z?¢^£Ýþ?˜yÙv-¢³?íWZä÷?°Œu#˜‹}?œË9ËH?¤+Ë–v7?¬$ÐÔJBå?£
*{wÇA?ívò®;?¡‰ñŠ5<g?œ€z¢á?'¼în™Ký?°'%£ßŠî?š` ;ººR?ì›"êªr?œ,ÛÊ#v¾?©èj`fµ%?•Xzíw?¬efñ'?eR¬*AGN4FGL J0731.5-1910c¿ÚÌ0X|¿È*VÀ¬'À9vf}ãZ®À;$(U{]@àšF<Ð@@sÀÁü?Ð`ÏM°Œû?Û¹1Å{@Ÿ€Á[ƒ@oå¤ßóÆ?´¬˜¿â·Í⠜¿éHL՛¨h¿ìÃ+c[¿ïè¶!å'ü?ï£êUsÐUNASNone3FGL J0731.7-1914c!?àÅTzx
¥?ÈÕ}ïÞ¹x?°Æü——k)?·Q
TJ†Á?ÚC—æ!mÊ?Æît¸?à-ìç
Z?Ëq@©
€?¨$ÖÕ…?¥g3š%Œ?ÜÁ	K>}û?Ê­ó\T?áü9*)Z~?´£Qdܪ?²¬_øÙ³?œ"pjCs?×\u­'[?³ƒ}è'
?àGÍkЀ?±x
5_Ã?´ò$5™ˆà?'š8¸É®·?Ú5kWøöˆ?±0ö¦]?Í5MCJ?Àx¦uÜ6]?®5sŸ
?©Õ8V2¼–?æÏUuÝ]?Á¯øü%ø?ȸ=×à@?ÇêmرÄ?³»'¹c€±?µ(¸ÛÔ&³?çZ‹È†Ó*?Èz©£kÄ8?Ԋá®8ë?³.êí²~?¸¨_<øð?¢§!ãò±¢?â¹ÚÒ¯Ì?´í«ŸU›=?Êñ"èº?¬¿ìŒØ+€?À?"€¾èo?¥bWî;x?ål"~–D6?²°Þد	MIXED4FGL J0734.3-4448?ïìY~Ò=À'ƒÌòŒyöÀ;ÔÈ("À<bZ¬ôÀ1@ Z¥@ð@>GÜ7£Û?ÃÍí^<Ì9¿Ÿ\1%´;ÿ?ÝC]÷)?ÿÈ¥Ó¹¥ÿ¿¼ șڿá \a)惿éQÓÂ_`Ž¿ÞÀúôÓQ¿á]Õh|Á¿Ö…Ôàík(UNASNone?ï#Ö䨶˜?"¬\óS§Ð?WmÛ¨^?KRø"'ï×?šE§¤Ö+?";¸Æc.×?íÛÝmGÅÖ?°ÈøÈ(?f>E›œ?oHq=™æ^?°o"jÁw?°^'ŽËp'?îøÛNòŠ?Œø÷M(þ?g•ûª²Òð?an
IX?ñà'~'Y?Œ}+5{?îßôÏË.è?~jÐowé½?iÖILšÐ?P8#ÁÝ®š? cQþ¸GÔ?~s*x[QÒ?î‰bøë?¢–B¨]d?gMF*ùT?^q!OáD?¥ûoí?¢OWã&?ëˆÁ‡@Èê?Á‹Ø÷äŽÇ?p™c6°¿?}÷îÊ-ú?ÁX.ÈÈä¾?Á]8""Ñ?í"5ðÒ»? Ý7ÆCZn?uRÈlk­?pÿ£9á?²	éÊ\Щ? C¼aR|æ?ì=oœP2?›îC%Tßg?"ÂÃà?u	ÑFÐe?»|>}1?œ^ފNAGN4FGL J0736.9-3231¿ÅÆ…ß(ÀL™Â´EÀ9RyaíÎÀ;'¦éä4È@ˏ¼ÈÉ@$§š
\à?ºürùO7?ÕÒýhv@¦¢‹°£@—Ž§x*?ïÿñ_{'¿Ú;ô¢Ô«¾¿åÊZâN¿+¿ê÷']gå¿ïÿíPÐÓ?ïñÂjÉ"UNASNone3FGL J0737.2-3233?ÓV3ÕçÊ÷?Án
í±ýF?ÔôHɔÖ^?ĽÎ	ìE—?×µƒ`ƒ^«?ÂoKÙ-"t?×ä5' ‰Á?ÉÏÝÔÃ!?È8
•Ì?¼Ö‹kÈ>â?Ü.xÛ«Y?DZpÙd"?ߜ€àv^?²nsKuK?͸ÃsN?®ù{ït‡?чeÁzß?¯õF8–?á˯e€.Ü?ªÒ¯i¦?ÇâbCµÚ?¢°SR4¶?Ðwp*p¨?¤+ËéU¢'?Â¥¾˜#W?µc&1«W?Û8:ÑYœ?NJq}ƪI?Û§èy¹?Åð½öMØ.?Âåˆæ‡Î?ÁÜ(@!>?Ô<75BÏU?Èz¹Ø±?á(C$öb?ÊðgY‰é?Ó!P1Æ¡?±]@ƒðéK?ÓC`…"l?³¢:/¯N?ÙÄlm³Ú?´3ïwõð?Ì™Y>ÿ?§èD%J?Ö=ú²
XÙ?³0D(iyÃ?ۂ8¡S™§?±ú(–MIXED4FGL J0737.4+6535?ïH«Ú'Ã@=@W:yx'À;TûwCÀ<Û:aû›@ Ÿï 3Ò@Ðh˜oÍî?¾¥õÝè(¿±Œ,ž™ˆ¨?ôn$ É8Ä@‡ó]ZN*?ïì³I¬¿ÒZž\!¿æø'}sHL¿á˜çBsB¿àØÏo>|=¿Öј
¨_/UNASNone?ïе0Ú?•ÿqŒJ«¿?="ˆŽÇ"?5m;ßÔÝ?v,\éø?•ü–N¹?ïȃ
Tì?sÍUÙßX?K²Ž/aª?Rx]|ºh?xH'u®Ê?pýÿ)õ?ï{A%¨õÇ?†­›'dþ?SLAÎ@ê?IÛ>ŽƒZ?ŽÆ4­0Ð,?†Sg·Y?ï²w?k!ýýg?`UËÆ?E€CÓ¨Ð?~ð¤]H?k;ðùZ?ïҜì¬?y‡''-?H'/ñ~Þ?@ÜæakÑ?s¡D4åt?y&%¾Š?ïv`í´+Ÿ?Š7ˑ‹\?Yq7)©Èï?f•ß9†Àk?9·^Ç#?‡Ì9‹W7?ï@ú"{ë?Žn|",®?ZäIû}•?YŽèØÊp¢?šiœwÏ?Ž "³~à?îÎü:VEº?Œ,Ôç{ä?}Ø=%?oPXËÍ^?žªt§)¡¥?Œ½
šµ8âAGN4FGL J0737.7-8047¿æ®îüˆ¸À8îÉâ6Á]À;mðwÌÀÀ<®rØœ@"E…sª?ûêՖŸê?˹®øP‰/? 33"'K?֓7_'·¨@–Æ4WK¿ïéZ¢
¢?ïödá+(£?êàöðŒÅv¿ßýS]?á¿ËA×e×ö!¿ä?y'"UNASNone?ï–xlDÄ"?µW`VÈ\Ò?(5ö¸´"Ú?Gºee÷É?Š
%•Vb?µXB†¬9×?ï×SÏòv?u«¶+'U?>aõ$]‡}?NE*ÕX5?roøфŒØ?sIÀ]¹*?ï/^eC¯5?ˆC}º2Cß?TCgø{–?@*F$•çœ?˜Ïüà™eö?ˆ(ˆ8ƒ¬?ïaesÝ?uü=+›@Ž?E²ó¥Ÿ•?8`øÐx3\?"*ëòõ?uƐލ&2?ï'Â}œ¨?©)ƒƒ™?@y㌧ü²?4ð{4áÊ?ŽGÂ]ôW?©óc/<h?ï‹u§L	Ä?ŽxšE'?Oú©>Ì?b	òXÕI?‹2eÎ~Q?‹Ë<€™*y?î–/UÇÌw?"®‡<tÐ?YLßèċF?URYLK)î?¥Ò£§>¼·?"ã£á˜¢?îrR€*‡¾?'¾1(–÷ÿ?R­6°qq?Q{§ŽJk>?¨EnKDžŽ?'¦%…•AGN4FGL J0738.6+1311?ÛW5*#Á@0TC^úa[À:¡1¦¿óÀ<TÇ$íS@wð¶6y@È7 þ}I?ÀŸ9Q´~¿šÛ"CwÆ?Ô6߇Ï@¸¹jyN¿¥´)gØV¿éyô'ô;§¿ç)GŒ†‹ ¿ëËì't¹æ¿¹` Ò¿ç†lªMFUNASNone3FGL J0739.8+1312?ï±H2ž¹?¨î÷Š‰²ü?QÃ<¥T½6?s×3÷2	ë?"ÆOçh>?§h*P'?ïÂċ¾BN?€3—9±?M¶>ûÇ?\`)63[‹?zæòF'¹;?|ê_¤¿3O?ïX-mmä?'œ e·Ô?fûÍ*ª	?o>²b©Eœ?'Ø­Ýq«?€p'¿¾o³?ïâĶ'ï³?NXð%j¬º?/\×ùÂbÐ?>ÊÀ½b?kE|¤€Ä?M~˜Kï?ïc6×59%?ŽGÎñš÷?`Öu¤?Xž¿B2¶?'~aëéƒÎ?Œî
 bDz?ïqTkßo?"ÀüòÊÜ?_Opñþ·5?ƒ}Õ	.—?Îü¼yy†?ŽOØ 9ú?î'li¾=F?"¹ý‰¥}?x°ä"X?{¤$"k¹?¤Ö—
雼?'ÍI²A)m?ïëäGÆF?p¬cØ
þ??KGë¹Lƒ?CL‰lÝ:‡?†Ðˆ,ڊ˜?oëhj‹ÝÄAGN4FGL J0739.6-4530?áŸF]Ì'ÐÀ&~gµñ¾õÀ:€ÄK"À<ùqp…¤@üoò2b@ùI¥e·?Ж@.l?Ê"hܸ?û‹Jì\t?ð<x{í¿èIg–Øõ¿ßܔÀìĺ¿æ¢þ)q¿äç½~{0"¿ïÿ}ž¼C=¿ïÿ·¥ôïUNASNone?ä—qÅÞ?ÊnpºÁ÷ ?³7Dy†A?Ã\ºòjý5?ÒLÅD\?ÆäîzF˜?çXÓú¤²Ž?ÈÏñ1'Œ®? =U?tD?¢Ïv¬KüA?΍ZÆõó7?Ç·
õÙWí?ë›cSf?¥âeæ8Ú?¡b ¸Zš˜?"$È!Ço?ºs×0[›?¡ÙW.?çù–ÖEÇ?£Ÿä@ıÄ?®æ—.D?Ž|}}NøE?Èb3='}c?¡ô×N½?àF-dãŠ?È&Þч¾?´ºQOFòÕ?¹qr°úóÌ?ÚEä1u÷?ÇpWE?á"'}ým?Ðß¡ŠB¨`?±‡ÁÉY<í?´Çû›IP?ٖèjÉ2Ë?УïµýIå?æèÐ5ÿõ?±²ÍGVˆ?²nòø(ÇÕ? §;\'?G?Ë%F*Ü¢ƒ?®@(¥jÒ?á<úëªCÇ?²=ٖ& ?·Ñ*'&@?¡ƒ!0Ìd?ב¿‡·;b?±Á< YÌ+AGN4FGL J0741.0-5226?ٟ
Š{!<À,Xépq'#À;wï‡â·ñÀ<Œ¬&dØ@#E†•…ã¯?üCïÉQJ?Èùƒ<Ù¥¿±P;ל‰Ž?êÀSAÆsí@¸(Üî'¿ÌH…ªÏL¿ï-¸À%t"¿ÔM›iR¿ßWçÝõ>0¿åÃcÍ.ò\?´å€ÝNêUNASNone3FGL J0740.6-5230?ïßÆJ›?r²He4%?!$-…l	—?Äüýù·?o'ŸÖÈlÌ?rfœÌfæã?ï1º´`35?®U²qÔD?_Á珝w?owž}r?—؍];¾t?­'¨Óô?ïž_&+?"嘵=ñ?It<Ù ?JWîVhh?ŸKZsl?"d
p3?]D©¨?•Ð,sh'ì?Põ	ÀT6?Aa¼¯ ëÜ?¤ˆ]?•Þf™þI?ïº?ø?}Ú¥è?2 "G€¡?+'µ®ûd?€ß4›Ï'?|"H2CS?îG"öéù%?»Éˆìð{?j4£3Âî?ƒñp"6Ž=?©æ­C{?»A\YOÛ?îg™±ŽÐ4?š(K s ?MßP1VÓ?G-}ØJô–?©è³Ú£Õ?š)"ê>^?ê½ç¡[Ò0?´˜…‡éÃÓ?l•HáÏ?kq)Ì×}?ĖWkÊ?´Ê~Ac'AGN4FGL J0743.2+4034¿ïmnK@:Yæ%cgÀ:ÎÓU}
À<~Güó@ÙJ¡!@|âąÖn?ʔ]Úü_?¸hšÉŽò?Ù‰@¢ŸÒå?íáH2ž¹¿ëzá³
Þæ¿î
# îø¿×,RÙÁ§Ö¿ïÿT©¥€X?ïÝe¡D‰UNASNone?ï®ÍcS? ?š(6'T5?`j÷3|?bBY»åù3?€1él¢¸û?šÏñ®ÿ=?ï4Ú*•U?¦c…dÈz?€ ¿í?'!»"Hڀ?'\ºÍ
<é?ŸJ¤O;b¾?î!´¿ "?xacèÊ¿?sûŠÊ?ƒ—®N>H?©€×N,Ÿ ?›µåŸÐ—?ïÓI,nÉ?`É{ïò'?a~TFŽ¼¿?Qˆ¹äÉ?kgbj¦b?WLÐG;Œù?𢡊‰?ˆ"%`,~?tx8qȱ•?}ÿ¤ƒ'?vD©ÙQó?€—uÈô
?î2ÂjѸ¢?³Bðª€?'xÜ^	?©§Õ"qãI?¤k"*$Ö?¤×–è)î"?ímPå9™î?ŸÐ¨÷t?‰¥¡(ò´?ˆI
HÀ?±`ıe¶?n¹Sð®Y?ï=Ñ»ZDÖ?ˆÆêk¶_ã?…½Ã:>ú™?)z…~Æ?ŠÍÍäàûê?á5Ðt‰®AGN4FGL J0744.4-1403?â^íð>Q@‹"ÞQZÀ:Qo­7PÀ;å‰bÙ@̀;¤›Ö@ÖwÁ½o?А^\¶#?×>š?‡@T¯ÕEAS?ôBñ—1Š?ï³ÃçJýT¿æÕ `]7é¿éº øžï¿ëÇC‹p+¿ã%áæåR¿ïÿÕ¾
iUNASNone?èæ5±	DD?Ár^âcŒí?œ2h êu?°úI~@{/?ÈàÜ6ª¿?¾b#Fè-?áŸy¸'Ï'?ÄÑ+'e[?±§Ã=ïß'?ªü¯"
½Ó?ØWÀOæÈ?ÉómdK?çDC	?¯Öl6H·?±~wÀ†€?ŸqŒ9}²Û?Ê0¼ùÏ?«+S•žû?åÈP©ï/×?¤$@s"ÿP?½ór†ÖË?ð
"ýõ?ÉåüU??œ"<5Ûò?ãд…O­?Ƴ躿6?¤Ÿ-
ê?ªç"‹á™9?×fxõµ#c?ŝ]Ç9¬?ÎíªŒtÜ»?é?–G-?Ã
­>MS×?ÀÐ8ÝA90?ãê
OsÜ?Å°—BÉ¡?àõå=±Ò?³f³))óX?½H~žìiË?¦ÆT|¥?ÖÂÞ'é?²§
–=
ü?×Ai~–*q?«®‹sZ"ˆ?Í&°0û?±x
‹pÍM?Ú+>tQX?­€±b°qMIXED4FGL J0744.9-4028¿ï×җ"WÀþô›»³À:mµWeA£À<f
w"@š—ƒê°¸?ü˺bfý?ɪ`;Tþ?ãÄZ7ƒúÌ@ßbц@X—²Ž³?ïz͑êØ¿Òê?yg ?ÂâÙ(¦¿äÆhÏÍ2M¿ëFz£4M¿àƒ ˆ÷
UNASNone3FGL J0744.8-4028?Ïq8T?º/G7Ä^â?àïx{ðD?ÁË´K#°?ÐhWä?ºeuO¸O?ÔÓ©»$Ù©?Ǖ@'§'»?Æ ð>Û¡Á?¿S´XÈÕ-?à
ﶪ»?ÆW˜º˜å?ÙÙ@&û[D?³îfÁfMx?Ù¾qo®ä"?³ÜŒÉ>²I?ÈМҫ€n?ª•§¨˜=Ž?å³ÍCâz?¢2SgűÜ?Â}.æº?ž¿0¼gM7?ɘ³œ
s]?¾Tšÿ"Ê?¼ôzï=Á?¬<§ˆ(i?ޞziUž?µýN0ê?Ú$gBÚE0?Á†:l7‹²?ǒ\â6Éô?ÃÓã}¤»?Í#Ûß0Éï?ÅëòTÏBÑ?âÒqϦ?ÉñΨ³×¢?ÊÌÁÇ9?°®À	íU?â1óøÆâ?·\šïžÍ¥?Ìoo??°NèX_
Ô?Ú?¿Lu?¬h=‡?ËLÕ	üi?°6B§|¦?Ø='?»µV?¯Vx¾ŸæÏMIXED4FGL J0746.5-4113¿ã}É6Í
À 6‰Å!ÞÀ:«°ÿç¬À<IP«éþ@8ñÁ"õx@›²ãízÂ?ÊÄ3êé?µ•þk?ì«Ð¾Hûq@^ðTf^¯?ïþÖ~z¿ì@9
ãˆÑ¿ØOr"¿ßó«z=¿ç›#§¤õ¿âà¥Ç¥EŸUNASNone?ìÛdƏW2?©À"eogä?aJ@†?Tý!Dóuë?¸œw{á\?©€ÇÞ¦i?æ†yæ\&?ÁRÞãêd|?x­ÏðdtÓ?€âÄÑÅËÍ?ґ#ÌÁlÐ?ÁPü`§ú?ímþ¾À?ô Î¯5?{ÅfËÁ×ø?sÒ,Š.?µS%G²þ?œÚ%Z?'?í;ÅÜvA?'"®:Í?w	€µr?TN…¯æçÈ?±¦!Biá?'2‰Ö]8M?琩Žcb?½×¼È{aÿ?rê¼-	¦Ü?is»³Û-?ГóRÑ?½®Þóî?ܓ$Ø@b?ÃÝÓ$ª¯A?zвM°8?‡[v•ªîù?တÔÃo?ÃÄ è'O?è
6ZZ?­ÙhI9Ù?+½$˜¨?  ùO+Ë?ÍÆg€ËJ?¬òš6®…?é0êÓïç?œDᄵsú?‹´ÕܬC?sP8uA?ɁU΂s?œ8]NµêMIXED4FGL J0747.2-0736?ïÿí'ò/ª@!…–À:Õ¹Nè›À<MÓÔ(
á@ Œ-·c?ÿÚÇ犾5?ÏÌçå,0?ªå Å®‡?à(È
Æ, @Rn6êM¿Ùù–#ÃS§?×ƺCÞ&;¿á'àb*íi¿ÙEÉ7ìÖX¿çÂb¿¤?h50ìåy UNASNone3FGL J0747.4-0734?î±Ë#KÖå?•§7Vw@?T¡4Ê`š?Kñ	+_.?¤>D$ÆS¤?•^Iv‰'?ë7Ÿ'h3+?½ýM¦¯Š?pßß
–|?w«ÇÓð€Ò?š'¼w-ù?¼z>èDo?íÄÔ5Kç4?˜Ð­êÏæ4?zÝÃñƒ$?zCÜØñcÔ?°7p{/yª?—«ñ5ûa?îÆwÆé'?wã8í±òŸ?t¹š—Sð?T£qÊ µ0?¡h"Äå?vڸǬs?삑t~yz?¬ïY¸¯¾²?nªÎdÅY?jìôÈfŸ?ºöétù&?¬oo­ð7?äÉåúù¹s?ȯԕ)X¥?ñ†FÓ»?ŠÇ—{(·§?Õìmïû-¼?ÈL•ÚÈ8?êˆt&Ý(S?§ÁèYXì?†vô>…ë ?|AG»ÝéŽ?ÄvÀ!~æ÷?¦Ð`E´ü?ìÒE>ñ?'6xÂ7{?"¨NÃP"ú?rS–o\C?¶Úe¤Û?'˜¢§AGN4FGL J0749.8-4420?å±/™ô;À"3󾩛À;9
£3vÀ<µ"6Æf@©ûv®] @RB<»r1?Ò娛•\?äÅýƒxñ@`ÔV.?òasÝó:Ë¿à†øaûó?UAª33¢ß¿»»Ñ«Xß¿è9']e5å¿ëUÛN¿ïÿýawUNASNone?åmÒ&ºA?ÁòÝ32˜•?¼'"@Øüö?µÒ¢‡ö?ËÿíD«D?¼Ñ[sš×?Ö?Uô[å?Êx—ýsnô?Äd$h{O¾?Àd]lí"?ߎ—ÖS'Ö?Èh
¾ŒB?èGæíp—~?®gJl(Õß?¶D
$rŸ?¡f¿P8ú?þ_Gtnù?§4×Èd^?á9Òé?¦–¨cÙ?Ò¿$Á^X?¥[.äiØ~?ŚnKBÙ? @ëXé€?Þ$ 7FØ?ÃɍKÇBŽ?ÅÓG¡e|?ºq!Ê~®?ÖòHû?ÃÎ`¢I?Æ%p‹ó¯?Å[Ö¯=Š?Íe}8Ì
–?Èññ×?¹Ì?ãDŽÐ<ï?Ëôðöµ?äU~4
x¹?±žO±¥[?À¬%@	
#?¨X/%Ž?ÍýáñæÑu?«G‰ b'"?ÑÈÜY:b?¨bp6ę??ÚâÄÕKeH?²‡	7ë#?ÓU(N[`W?°ÐW¼Ú…UMIXED4FGL J0750.0+7140?âff˜T9@>>A€ÓÏöÀ;'u¸êÀ<^£ƒ'gM@ia ƒî@™æáK	?ÂZ	‹Å¿Á0'B]¼?ð֑§\л@QPiÏÒ¿æ{¼n°·Ã¿çýՃT´¿éØ·¡Â]¿ä´>Kë¿ïüž…¿ïï,"¹ºUNASNone?ïÀÜ䇿?¡Ì?ə'Œ?c¿ã…úï?g>gé!,þ?u±œOku?¡º9G†?ï~eîhË=?'å5wÄ?rU8Bpû±?ƒæ³¿fÞ?‡;èM+¸Þ?"•[).?ï
1kÝɟ?;ÝbŽ?v®ÉðçÉ?xýȔm-«?˜® ©Ý¯?ŒÙ~!s6;?ïbF\8m¸?u6¶
®?t?|• x8?gn1â'^]?‰#غPOL?q'áó'Êœ?GŒJj?–L´/d?€LQÎe?Ó±Ž
?zž[ÏLlŠ?"ÏD³Œ?î³Ôõ¡i?£\7äGè¢?'ÛqO(L?—ažÆË? Zâ(?›¦~q""?î]‹ÀÔ›?–=S®¹øp?Áx4^÷E?~¦¢ù5&Ñ?¥¶åëèØ?"6-?íoíQÍo?œõÕOÓ1?¡V!¼ìš?"º./Ug—?§ûÔÁ¹€?"6lÄ;"AGN4FGL J0750.5-7519?¸ti"ô7XÀ6ŽØ
±À;!n
#ÔñÀ<wñ8¼ßð@–'âòþæ@«Âßä?ÓʤzHF?ÛÞ¨éϒ@}€Ú…ó@Œ T‰D7¿ïÿR@>´q?ïû¾½?'?ì"}Š¿èîê.¤¿á‰ ]9–¿ïüö@
·#UNASNone?ï'H)?€
üÓ0U?c6‰?_°…Å?†àDɔ¦C?|L¾ªä/k?ïŒlAò"±?ŒE!ì;?g›§n«?qÉÄÌ!¨?†þ¡Lë?†‰îõ¤Y?î¤\æ,f³?"ˀؓ»š?ˆBÏÙ'Á>?†‰n#¡ß?ŸRûS³?''ô ,Y?îJ"±'Ì?ŠÇÆ3ȲË?€Šü
cf?q¡aãïƒÿ?§3õèqë?‡ø¤d.ñ?ï,¼Pþ /?Œ9=4cO?uV­%Ü:?q£´«
úZ?•ʜ–°"?ˆ%Ò(›¯?î´vUXd?¤¼Œ½š?€áâIgþC?9™v*¡? €"ƒ¹®?Ÿ¹hÈ¿—?íáA2<b?›Õ¿Ð4í?'ï2…†?‹øËLQä»?©õVŸB'?—%»ÇÈù?ì-À¦‰þ,?¤\ßìô'`?Šý}Q‹ú$?†÷ãgH,¢?»2K#6]W?£'pÀq.AGN4FGL J0752.0-2931?禘ÙçM¾¿ômY4N¼&À:¼&Œ[ÃÀ;èH÷À–^@]6fïM@]<9Aj?͐½'h?æêúêíID@^Íñ?ø~…—<¿Øy|ӆ¿µjF€þÿ5¿àùI—ù†i¿ë÷2ú(P¿ð?ðUNASNone?ÁÂUÙ¥?»ï¹*³?ÔQÕ­•?Ëê
ù'.?á‹Á±)œö?Ë©÷H).?ÆñÎ~f…?ƨœýãV?ÑŽî' £†?Äz'Dû Œ?á|=œ?ÆÈqÆ?Ó2 ]¥o?°õäÉás?׳ÍøE÷[?±×  §'u?Õ'©¸ß?°;"¨î6¯?ÒHM»cˆ?ªŠ¾tZó?ÙÅ~¿£™x?°znpj?Ô78ò¡?«UÀ£8%?²Î"õ8ÖÕ?±ä!¾iþ?՚ñÿjÆ?ÎþìLÍk·?âØ¡<C?Î7ì¶!9·?¥šJ®íÉ?®7ýŒ¬•?Ô/óOdä~?ËV]h՛A?äŽa­¢˜¤?ʖštª?Æ2¦þ(†Ô?¨ßðɉÔÞ?Ü9³CӃ9?´ûZú?جù=9]?³˜ø‹¡Ç+?·¢×òð?›È	ù»Þ·?ÞÅK%dµÚ?¹ŠƒÏá\Ú?ÛQÿ
G*?·Äƒã(MIXED4FGL J0753.1-2624c¿Ï€¸L7;+?á!l—¥À:ŸËz½5€À;÷ÏdVÁ®@ùáxÖU@1ìVuX?؀ÌÄjÁ?îܘQšýG@4' ÷@f"ÄB¿ïÿñò÷?ïÿ@Aä{ë¿â5¯^ý¼Y¿íLE¾P2G¿ïÿýaw¿‹4J_t¯ªUNASNone$?:ÇëÖA?»Ãmr¡ø?Ã5:K¢¸?ÁIXȇÝs?æ‹b»¥ÌÈ?Ç2o|BNb?ÑÍ&4µ?Í^k	'4ç?ÇvD™s??ÁtS¨¯¦?á"[ÊÖ?̺*"|t?ߞ¤iðùA?²øè·Û?È+b¤ìÈ?®ð¢.ûõ?ÔKªCÇ[?±;MÏÿm?Üé¼£2?«"ÙJÿç?ә ãOp+?«,µ+û™Y?ÎúDó,»}?¥†i¾š?¸j5¿œ»ø?´oË}!?Ç"7ë?Ä¢Ì{̳?ç*7:m¨ê?Ç A*º
J?½®SØø²·?ÂÏÑ,5›¡?ѯ¼#dç"?ʚTN$¿í?ãrWs.uß?ÍÆE/pAB?ÔÎò±e?³ÅüwU?ÐÚêÿŠ0½?¶q×WÀ0?ÚV"àÄjB?´Ä‹ày'?É[!à`¹?§‡¥éB«?Ú²ššS0‡?·f[ßNڄ?؟Ôu|r±?´ì3ŠëËMIXED4FGL J0754.9-3953¿ë8'Kج»À?Ë~3ÓÀ:¢rúÉÀ<ÄxCÞ|"@Ž}á,U@?Qi›?ÌEú
G¬'?ïþ¡€Ã´Ë@öÇê弈@WzK˅z¿ïÿú@ùDz?ïþ¯¾3G?æiªK¿Û©q="ðÀ¿ð?íáŸËŒÜUNASNone?¤Ôð
S:ò?°Us¶"V©?ëb
Ŋ?Äe€[ô·;?º…7.aߐ?ÁSÊ­bÏ-?®Œ}#?µg:Gø²Ç?ä§LµÃÏ?ÆB#íV@e?Òáë5 Pá?ÃÉ%£Rªó?È6ÜQ
o×?­×=ÛV0?ãÄ3ˆe??´`Kªw7?ȸUac.?¯%4ʐq"?ÌOá×Bhþ?±±¹éÐ?æ4‹d‰?¶BŒ_^?µ»á1Ҙ»?¢¯Xì¬ñ?«pz*W[?²Þ1a‹ð?é¨j¥§š?Çÿk:`¤?ÂzyáËë?Äõbm2ˆ?žçß¾:9—?®è.I‹Ü?åDBó3ƒ?Ì
<ޜ?Ӊi~QrA?ÊÞÚB£‹?¾›Ná ª–?§©Ì~´–?åmSSþɎ?µÑR²±@ö?Êý?4"}?²›Zçrº?°\õgÍN?£›2÷©8V?êºyT™y'?¶}oª{?¹Ï?òøõ9?¯/1sØyPSR4FGL J0755.6+1855?Ð%4õú\@6_ºº{'qÀ;]K´3xÓÀ<¡ÊVÐÇ-@´¦M@"Åyò4e?ОÖd¦à?yT¿"~ÕÕ?°¥ô›ÈÈÜ@~ù ?ïíL~Þ­J¿Þÿ<÷S½¿é­Wâ1»¿»uøÀ·¼¿äd¶Ê,¿ðUNASNone?ﶭ_¸ç?úË®È?MÎ3ý¥?`Fc»ãÚ?€"{ ›ú?Ž­@*íˆg?ïÑ~,«¯œ?smÎçèˆ?D¼3?NÛtrøL#?tÀG9l¶¡?qÐ5ã?ïS`—;è±?';6¥?'{?cFÿ¿ýG?cç ò|&r?"+
'Žló?jë¼í'Ö?ï½è}¯6?_4–GóK?N<ï÷KØ?2äQ¾Û'Î?}DYßbF?^ åþJü?ï¤EŒ§}?€d0"®?P7ª"'?H¼V䇱Œ?"Úõû€?%áÜîsâ?ïŠ)@¸yP?‡'į¶«<?R«tL(Æ?`	í#Xƒ?‹ A>
ׯ?…¶(¹:?î·ºšSÜ?2ǓØ™?o£D¾x¹?n:ŽQ«$?¢Š*J]DŸ?ŽÔ+v–Ù?ï6ÈØ1Àþ?|n^9"žÐ?dp¯D£"?T"ÂÍÎ=?–˜Ï™ÐÇ?{Æ	ÄßùAGN4FGL J0755.9-0515?àêÏ´³¦`@''´·,RÀ:‹kÙlîÀ<³'àÚ@O—íÇï@ðù'7}E?¿µ2&mÒì?¨VL_KŒh?ãmjñ¢?ôäŠ$[ª¿Ïl?XÛci¿ê-Ôï°ýc¿ët·AË&"¿äü¦¯+Ò¿ïôèà(Ê$¿à†HNMjíUNASNone?ï™Á‡D?¢JQq‡Ž?}f0]‡"?¡×¦"3Œè?u¹¼"vñ?t€f«É?ì8ú1NÁ?½I›e²È{?¤S|Psåõ?¨êçðã¯?´pMqx?¶ÄJŠLP?íD™ú‰ëÉ?ŸŠ
"(|¦??Ü?Ú¬!?"±GÅs?­r4Qd?—'W"t˹?íםu=¼?±5qÅÎ?¡Ÿ@Þ¨¨'?‡ ®ÔÈ? æçÐë1À?€'Žàõx?îÄ"9»¸?©"R6bûh?›èœ¤‹_?¨j?Úx–q?‡.¾'1?‡§íB®¾S?磤'úw?Ëw⇪Ù?ºº±jç?Á'ú"	Y	?Æ ₟5?Ä£LhìÜ?ë'±qžö?¥ 'î•?¨òRUÖ.?›÷ç¥¶¿?·v™h¶·? LtâO÷×?é´ÌŽA)t?«äÆ5%s$?¼^}(ö?§Þj9FØ?µû‹œ°ï?›ži»o'6AGN4FGL J0757.9+7304¿ì_)ßU@>¯½¯ljÀ;Ï1_œÉÀ='òH‡XN@ šj$"?ûÁý¶y¤1?Ôp†yÇ?Îø" 5ª‡?÷*ÑJ
M@°sAI?혬3Ð%¿êVg€AÙ¿¿Ñ
7öçRŠ¿àëL4"†¿Ñ`Îvðø%¿ïÿî,˜å?UNASNone?ïD¦žËî½?±¡êökr8?miR*w~c?Œ|¯G
­?"¾Ý?®»|~'è?ï'Hο¯ó?Šç™Oôi\?fä\"`3Ä?m!­Q—ÚJ?‰´µ*¤k?†+¹^‰aä?îëP5w†?'¤'H¸î?xæÌÅ}L?€UªäÀ?œ\F!Ù`Ý?ŽÍ4
O}?ï"2<à?g՜vè˜?Smm»u.§?==ǍYäe?ˆÅÍ	d?g#ÇÔl2Á?î±;©Ê?¨fԈH‡…?y×MlÎ?€ƒwþ›$T?¡ËôZ'cC?¥"Ì.±8?îä$«—.A?Ÿ±SÙø­œ?s,oEe?œµzš(Ì?ž°i¸Øž?šì"‰MW]?í«"ýtÏ$? kßn‡iŽ?"1òӉ	í?…sh‰T©?° ©º@[¤?ž˜à«ÔP?òG?ˆ•ÃN³g,?cNÀÔ-V?Wè3¤ù ?¤ó+ô4 Â?ˆF—£|ÍAGN4FGL J0757.9-1514¿ÂrQ²‹i;@ë¹]"?•À:?eóSIÀ;Üèi
…•@T'ÊtX@ÎíEé]?ÌɞÄüžÍ?ÚX™Ÿ"ðp@
2Väé#E@w5Êè2?ïû™3BL¬¿áŸ
='¿é¾kÀÃT(¿îÔÚbaŸ¿ïrô^Œ'k¿ÐÚáŸÌUNASNone?íKvGHئ?´_Ü"o‰?"r–®)^ù?£sMtÄ?°‡¨w?°éîDŠ²?áªûë ?Å eêÚBÆ?¼Ð>õ‡?±Í$:»Ëo?Õuø§h†Ÿ?Â×¹³dú?ê°5gjó?ª¼›uh—+?«XÈHL­ª?™øQKQV?Á
sAÊ?¦]©ç5'?ä¶ÃÍ?¨³ƒ|V$À?È[t1¢†Ë?¡¢q&ÛLr?ÄÉ|˜#o=?©Ï'I^Ýu?êzðîœ£?¿›A`-ÎV?¯ñŠGFYŽ?¬Šƒ­ó8‰?¼/¶UUá£?ºþÞutT?Ð"àþz?ÅútxÖ^?ÏÂp^-?ÃC¼'`R?ßüFöÖÙ?ǖü]€†?åÔ1="?²¹³àeu?¹u¿Øo?¢ÃXU'¿Ç?Ïs.~v0<?°‰ ǀ±?ÌÅØJôë?§"‡ôÇ
î?Üђ'4Í?»ámîšþ?ÔˁIQé¾?»ÿ‰eMIXED4FGL J0758.8-1450?·£Ôz˜@sÞ¤e¥vÀ9éɼw4À<O‹À@Y{SJ?ý–ç½éÚû?ÉÁžÛÍƝ?â¶ÝÂhoÖ@Ÿ=áâއ@rÅë‡"?ßcøb|ÌÚ?ïàuöý!ÿ¿Æ:'v_'Ç¿äÕub'¬¿î"0Akˆ¿ïÿŝƒ‰UNASNone3FGL J0758.6-1451?µ'ÙØÙ2|?³O³M'˜?é¹øÌ&?ÀÛ¨^û°\?¼¤N`W¥ü?µ…Rb«úM?°£.Îâ‹,?´5j¯Ÿœ?æw%ëò«?Ã'®Þ¶j?ÍÑÐës¿?À€ÉÐ)^Ú?ÅmåKHÓ®?«)QJ.ÿ?æœg@?±¯(¹l£?'E>ðÎ?§.)ö'÷Ü?Ñv¥CÃ?¤®<ßð®?á#D<½B
?¬FÑÖB+?ȅ¤ˆú©Ä? áFé^Øò?£óiHâ՟?¤a)ÝìQD?éJÀž9?ÉBÖ¶§ê?ÅØ%r¢¬4?ÀŸW|FU-? L#2ùÁ;?¦/ÓQÉÄ?ç®kÉãÊ{?Æ@ű¿D?Í3H²eÃ?ÄÔ¼Ì?´Ÿ[8˜Ÿ? Í¶^yǒ?èÔ;ŒP¹_?°{ ƒÝ^"?Â_' {à÷?ªÒX³è}Â?ÁÙNÒîFg? u&Ùľ?âã²Ùuk?´èìg¯­%?ÑKòãžË?°†‡r×aFPSR4FGL J0800.1-5531?áúÜÔúHÀ*@!ÀD(NÀ:Ìá*?À<ªGfÆÞ@ï°oÉçj@ÁÅg}¾?ÉÄ
'?–%"›ìÁ?ÑXŽß#@ÓÝ¿¹>?ï"¸Ç\J"¿â@!X?\¿ê
…/J¿æBM'iҿדrãø7Š¿ïÿ'ö֌UNASNone?ï'S›ÛÕ?†Ÿ¨z¨ª¾?\»óx\?TçfÉ0Œ?‹ÓšÊ°¸¦?…ñ*xo@?ï$-xM‰? æ¢u)Ž?cý§	.~?m²4x^1Î?˜ú­¾fC? =?¶åŠ?îÅ2+BÆF?ÂlŸÜú?um
)÷?q¹‡lu? ÿ<þ?€òQî>Ÿ?ïÈfœÓF?ttq …?[/5æT|ì?BË³«C?šÓÿ̆p?sÙbŸkòk?î¹39"?šd tœb‹?r°4¥IK?iÚÕê
>?¢ȇWr?˜·æÄq?î´âÓÒÙ?´U‡é:c?pb|ÌÚ8Æ?~ö°3VŸ?¬Xb:ßYT?³ }Ý5?í×Ù"ú	?£rY"FD?ˆ¡ÈÇl?ÔØ/?´ÍÌýÏB+?¢¶a'A ?í+ìE@¯{?"óÓæ©?t:"Ò
Â?d1˜£*_ ?µ\ôˆ¿Æ?''ìæ€zAGN4FGL J0800.5+3715?Ù{Ázf×@='à°«À;¶–ʞÀ=jïVd£@Q±; è@¤+eßWê?֖©ÁÍ?ïþh@0FÅ@
ˆ¹w…s@dCðš²H¿éŸù8¿å";‹ÇI¿ÈE/‡­¿çTÁ£Mø¿ìrô´rbô¿ïÿ»×²UNASNone?éwwàƒ°F?Áwþ\ou6?Ãîdâ'Á'?Àjô9<%?¨Îîm¹õb? µGÑÏ
Ø?å»zÙ Sn?Æ
{Ö1œÓ?ÍÙÕzV™{?ØV½?ÕÈ?¶p~Dÿ™?ª–¾8ƒ€Þ?êÃ3XAW?©3f¡ÚÎ?³w魙…ì?¡‡áÖLï?¶n~@€VZ? }ûvà/?ç‡P¿
Aw?°(åîB#¢?Í\ÓI2¾?¬Ï§¯A8?¢§Ú' Œ?•ƒ.6š[?å.Z蝧Š?Çdšðlö4?Й
$"@"?Æ0Ii*ø?´(ô)?æá?ª´ U s?ÛI~ý>¸*?Íþ}œÁtÞ?Û|Hc=‰?Îôí怅ª?ÂtÕt¼™?·_Uä?ç=QKÄq?±š9ä%¤—?¿â¶ùž3?©MO!Òíá?òõqlæ?¨š÷t'ó?ØíéÐÇ5è?ºÌ‰cŸ`?à‰þ›üË?»Ü(kô'?·\ǕNˆ?¬¶Ðô6MIXED4FGL J0800.7-1059¿ªþØÙ7£·@#ú£iüóÜÀ:Qû]ÙÏëÀ<9¬üLí@×Õë™"@ŸNìő?Æ	[ˆçÅ¢?ÅAòé—ï?ý'-K6?ü/š.êÏ¿ï²LîÆÙ?ïÇìÞe%Ÿ¿åÏ/!}¿åNžsž¿ïö§ý	«z¿ï+þ¶~ØUNASNone?襙Áÿáš?Ä¡,¾'Å?¥ˆ´E̦?ˆ,r[÷~?ËTç߈øH?Ä£ÓÆs ?ë$÷×Ι½?ÁÚÈO±æd?¯†¬ÏMÒé?²ß^䀷d?·êÚR<%?·¶ù€ÝS?ì'ÃkúúÞ?¡Fß'´?—¡E1"çÕ?ŒƒRcàˆ?µ"U—=?ão5íG?ë³+EJ"U?"gÁ"¼8v?²»ó•‰J´?	ß	·Ð?¯Ud'ØÚD?…Ï@Ç%?â¯Ñ"Iã?āà³g(·?§nû3$‹? '¡RÍ6½?ײ™™³^«?ķ兼~1?åì¹ä_2?ʧ"2úÝ?ÁN-4—?ÂÐIó­Ñ?Ç. V9?³ŽÖOµþ?é–­^¦?ªª9ŋŸ?¨Mî7?–ÚSK–&T?ŝϜq!?¦dÜHvÙ?ç…Ê—	é°?¨ã—ì$¾Â?ÁìP^ïH?¥}TÑÓ?¿ù
‹|Óï?›jã½@AGN4FGL J0800.9+0733?풼È?@Õ@2ÜJ@•òEÀ;~™Pž~À<éö\é@ Ž¨‹úʌ?ö½õ<ó¦?ÖHì'õ"@?げ©@ûA3¦ö?ö~ÌôºÒy?åè阵n¿ïÏYÚféC?ïÿÊ»z"ò¿•Ã0}¢¿ãÍé,~ä¿ïïá9k[™UNASNone?ï±t_?/L¶?u1ËÛ/n?qÉ¥	>4?—P©VI9?›¥´è§	I?ì'"¹à®M?»"}'¹ü?¤q˜(^K?ªk™ 	ü&?±>§ƒñ?´sdŸ¾?ëžïÇx¥?ªPE‹Ò?œWØʀ?"ìZ™?»ò‹'Åe?§ •¬¦?ê·¾0/{K?¡'=^24?£ë›ú.ö?ÆH™ä҄?À\X±z"? EËT«?îL»#Eï?ªŸKp|ûå?ƒÎ˜f<?€¨§%‹¼J?¦@Ê)í)Þ?©y•%î0ˆ?è+äj«Î?É»{…v:ß?»QÑY?ÁJVðýƒ¤?ÁÅElÏ>Ë?Á]¥¢'dí?éôG"†ñ)?°äÙ½Xã? c¾ßVð°?–†,ðÈj?Äó¿!_î?¯øýAߞa?åñÆsí7¦?´^±ÊQ˜/?ªxŸÁ)j?£ŠžçŸ'?ÐÚ¤ˆ~G?´²{ÈæGÏAGN4FGL J0801.3-0617?ê–zrY[2@(èä¸{ÜðÀ:ŠS±WüÀ<s'È@ùº=S³@ ƒn—?ĝwI¸…Ã?œAí¤ø?Ö–­V?ü»%_5?ê?'—•¿±¥Ku쎿í3Ðçå¿Ë—¡ò®‰¿î#f!/a¿ïü]°	sUNASNone3FGL J0805.0-0622?쥫¸Õõ?´ì¯	¾%Ý?ƒ3rc'?z™Çe|€?¸sŒ1Ú¡)?´oiô>ª?îâ
!?­Hë+¾'?~Y%ú%Kš?†{a!u?¤C
Α?ªTúQI²?ì›Lç[»µ?¤qjä?ÿ ?'û|§_D?ŒøSh?¶…™æf>?£#ap¦u?î4ïN¾V?‡¸©Ró®?"»ìµyÀ?zLHj–c'?¢S·ãÃ?-\‹ZŠ?꜂>€¬?½ðÓW-?•6Ù¶Gõ?Ó½¬ÉL?ÂçÏᡓ?½
=¤-úÃ?ëÈ¡áwÝ?Á¹{óQ­?–´¿«Ü®?¥•¼o{p¶?¼
ÇÃ{í?¾daÔ[a{?ê)&34N«?¯~|STê'?žÃ´Ñij?'"ª@¨32?Ã<&™>?­®	q¦ˆ?ëC.vò?¢€Ûî¹í³?¯"S?›ßå—ï¬h?¶^½=¨?š))!¿öÙAGN4FGL J0802.1-5612?ï+ñ-‡Ö+À*kQœIwÀ9ÑÈDŽŽpÀ<Wí|o½'@
¤þ&¶ù?ÿ¡Å'U°6?À]¨½#ž?èMàÞ|¢"@#sÈ:–ÔÃ?üüo'ôn¿éÉ9d¥œ?Ðû‡n…D¿Õ´`$-ó¿ê$ŸANSö¿ïÿýç!é?èAôl#UNASNone3FGL J0802.3-5610?ŸØD(Ў?¥bu©Åù®?íÌhÈ㫃?²
U}絧?£MiNÔø‹?¦È½©±NH?²øû®%†'?¼s*D!B?ë€*Cb?À×»àÁ?±³ïÂVb?±rÙMz~?ÀŒjðAy¦?ª¼¤"Ä ?çð&Òw½?²0õ§j?¿eóYNÑ?¨ÎÛ¦ÖÚ?¸®¦ºø
ª?ŸqXƒU?é²zIøÇ?¨m÷´"ã ?¹½ˆƒ"?MP&úù?§HŒ­?AH?°y)ûe·K?í¤õ©v?¹>=*Ì?§
#ø)]L?ª˜†Ã!?¡Ä(º8"?±9Ry?í;'…ܬ?¸oEg
6g?­H!µ#¼?¯"Œ¡vxP?²žIN:?¢áþÑñh§?ꌜ'‹?®š U¥—â?¼©QK2j?§èÊH&ú?šMµŸÇv›?‡AÖ(Ú?ë~[¢èø§?«8ëÀ<.?½yµ4P?§ÝU…=x#PSR4FGL J0803.2-2522?±Í"Ç…Œ³@ùݧ¤À:ãhšô­À<0ãs\@…_ KúÕ@ª¬Ùè>B?Æ2šÜ垫¿' ƒ~áB·?Ð0¥Nفç@b"¼î]k?îR¼›&b¿åîs°Ñă¿êM=Ëg¿Û!L€â¯¿Ö—†"iÓ¿à"ÈŸ@¢‡UNASNone?ê¯i§¹lô?·CׄÜ:?r¢]Úq<?fj¯WL?Ä­Frˆ¼/?·	pP8ìJ?窼O.Äí?à ÕdÃE‡?…)|9Ý'€?Š‡Sõ4Dâ?Ð;ï	Ê?ˆbô…½3?ì¹=eˆ'X? £Ù¦Õ
?{êdáÊ?o»Wß+ö[?¸wn…ˆ"b?  §DÞô?î¸çtB$?{Èè/·zA?a‹¾÷atß?F¨åm_?£XÌÉí€i?{/n'eò?äÒÞ#?Âî%}?ƒª/?uoP‰Ÿr?×Wƒº_6ò?ÂØèP®:³?àÔ잤?ɓp†aÒ?†§¦–ön?"¸tŸ:øŒ?Ý¢ŠÃVÆ$?É&X0
 ?è$¿îÄ?°ќ3_¥?‰MB›Ã
?y¼Ø
?Î^˜ãL|A?¯Š		½8È?ëÆú		ض?™¨(ùT‡o?{Ìxæ/D?k#ñ,˜±]?À´D/°?™ vèÛAGN4FGL J0805.3-7425¿×í¢ðÁõÀ5QŸ<pɗÀ;8rǝ¸ãÀ<‡TÂÏóÉ@x4`YÜë?ÿO²ZZ¿i?ӊÙÂÿn‹?Ôb'ÁÙ'?üµ]åŽd²@T"Uð¢¿ïû¨b4R˜?ï$‡nÊ?­âcAën¿äO
?¸¿ãÏJ ¸æ¿ïú;e0ÜAUNASNone?ï™c衃b?~ÐO	9Ñé?Zܺ'Q¼Q?Mõb¯·ÄÙ?†Kn{NN?|ëPÊ㈏?ïŸõ§ÙÆ?'ñ¦!L?`OÞcôÙH?dÎû­`Lþ?"&Êñµ¢T?€&;Bì!È?ïm1s?ŽÞߺ^aê?xJßô3ò?v—û'îø?˜ézaØӏ?‹§ÅÐ?îL'°f8?€Š;v±^É?|µì癉®?`ȃZ4v?§ bTÊ?~ÐßX!?ï<àîÂÀÚ?ŒÑƒ¢°p?j´\ٖÕ?^¯‰®áž?•
V|ì?‹¨[R?î߯ÚðôA?žýFÑÆgË?xIØDÞÙû?†‡"äÃÈô?÷Ž‡æÀs?™šìÒ?î Ñš¤Ê?'õ¢®ì6?€ªÊf9žž?~y"Eòþ?¡È3ãnµ?ÝÞì)Ìg?ì2ë\&hí?˜¤À&ß?…†*ga×ï?u%³i¨]?»·ßÑrŠ?—	MÂ7AGN4FGL J0806.8+5659¿ìÇ(B´'@@O+ý´Ì%À;¬sè/(âÀ<ôe;Ãûm@ Ó{d¥F ?û¯W™?Ön5Ó £ä?ÅöRT"Ö?ñWE+ƒ;‰@ï¾Î²U¿ïÿêf:Ç|?ïÿx†#›¿çöˆ‡ù^%¿»ñöýÍË¥¿ïÿ‰î*ëf?ïüÓZ…‡"UNASNone?ïÉjƒä?s5¨"Q?eÞv¥É1É?gâe&&±?p[¾íéŒ?hñÃÐ=?ïµëÃ¹ÿ?~òb(ü@?XLk/zI?b.Û´íð?~êl"ó‰ø?x«¬­þā?î(ûLo¢Ù?š_K!ãëÒ?ƒÑÑ|àu?"¾WÓ¡^Q?¨{ÖÙù­—?˜;ú_ÎC?ïƒOƒ~'Å?q¦»"'®¾?j
'œžM?WfTÿ¨ðŽ?ˆ©~n8ûq?nÛì»WÁ÷?ï£Qse'?€ÖMõ™Y4?vcW°?vŒU©Ž?xxÑÉÈø¸?u` |yY§?ï7'G}Ô'?–Q—áÙZl?i}	Eñø;?v"P•¿#?•ëußt'?"€›h›¬?í"½.´?¡á¸ùþ€›?‰!ޔMéé?‡,¢‰ýü7?´/&F+V? ‹cÏFõi?™M0?=þ­{?za®‡nŸ?t;F7QçÞ?£8àj¤?Ž07!Ì¥ØAGN4FGL J0807.2+3312?ïY;R@=q
{é…jÀ;{ë^ˆK"À<Òâ'0ïŒ@{;B `ô@¡E= ó?Òå–È.›?Ò¢
a,ë›?þ$Ü=ƒN?ù<p>–©?ïþ âx°–?ïí5€†£¿Ë¤è'4ù¿æaµ&½Ú¿à_•'Í~¿ïû…LXžUNASNone?í‰uYÉJ?Ã+ÛÕB+
?'n>mÂ.ó?™˜x*ŠÍ?±feŸ:D?Á¦ñ³ƒr?îçV™ûÐW?™ÁÁ·ã	9?ˆF\´§œ?‹$"xà?–ñþk‹U?~*K…?î1âÏ~¿	?˜Xi¹Ý$ì?ŽˆúéTh?‡¶+ÙIHN?¥[ðÈ}ÓX?" Œÿ?íi	¾DÊ?'{¥QƒŒ?£¢â{\X ?‹tã*'?¥ÄLé›BD?"ë‡öM'?î¹òâWšé?¤šÓË|f?}Œ7ÔS9?Š ã|öýv? ¯JÝ~2Ñ? j‹–ÏúO?ì꣱íŸ?³;J‡L_á?¢Å›F–2?ªqý™ÑÖ?®)—ù½c?¤¼B lú-?íԛ•·?¡œ­ø°²8?™ažWMØ?'xr?~X?±2¿I—Ô?›"-Þ!Ã?êZøwܖ«?§Ü,çï±â?±)
áh?¡‰0Å¡ÿ?»ÿ2:9â¥? aÛøx4AGN4FGL J0808.3-5121¿äQÿ^ùÅÀ#ñÆónøÀ:p1ÆK©LÀ;ܽ:ˆ'
@h`©
*
@
	Ö¶[?Çî•ßе?¹–UGì?ó~5Å´ª—@G+ÇYx¿ïZ쐰½?ïݍyЦv¿å©mƒÐ¿è×_Y¬Å¿áWÊÂ0'˜¿á2€óUNASNone?éÞ?Æ ?º-<±¹:?s^­R
´ä?füð#9¦?Çí–0È9?¹õ(i3Rñ?íVýÄ«/?¶¬ÅÏMGÁ?uvvOÌq?xïôhøß÷?³ðªtù A?¶$–íÇÆ?ì1ƒ$"'?¤ƒ¡öån?‰£ÖÎF÷?€4 ÛýK?»?kÿò,ò?£cGvVás?ì(Ÿ›ç&À?5ŠË?Œô"A9%þ?q!‹¿‰?»p¹{Œ=?˜E~á¹?åDëED?Âñ†—"5?èA/Ôm?u­x¿=E?ÔæçlؒË?ÂËeªºåU?é؞‰Ø?ƼºÃ{?‹cÓáf†?™ßÿ}¥Òu?ÆçH›q­d?ÆF¨×‹Rë?çH>[
?±þßt"Q‹?˜ÑCA,Ìæ?ˆR¶ä¶¬?ÏÄÞ+nî ?±a±$¬…û?æj÷Hó±?¥C%ß+¬Ô? Ï‹Ë©ï?¿œì	?Ñ SÝwÀ?¤íÖo~aAGN4FGL J0809.8+0507¿ê‹µÞHË @3Áõ8%á;À:ˆ$?ziSÀ<@w¯<™@iIºß™@…N{ŽØ?х¨á`,»?ëtm$ƈæ@× eeµ@	ÒG6u\ù?ïþš¥2T¿ãœ \–ÙÌ¿ìÞî7€ ¿ë7ë(Øf^¿ïúžâXÐ&¿äC<àÛødUNASNone?íð쏓cþ?¿…4n?ªÒy<#i?¾?fG\¶?ˆ|ž66rÙ?"¿4î%5?ãcV¸¸1¤?Î0cÚäD?Ó=˪/`b?˃â	]T?·î"¦T?²Ã¹ªe«?ègàœbvÃ?¯½§ß»9?¾Â<6MU?¦îXýZ$?¾µ8àµü–?§ü¼ˆÜÂ?åò¼å<ôí?«"67~ÚA?ÎWìäLù¶?ª
H,³u
?³º?4Š¯?"§¢ÿpyj?í–'"ÜÑ°?·mðbi°?°K¬*™E?¶¦ùo~NK?ˆ1`—'Ï?ŒÍè¼Ó–§?ÖàÊÊWì?Ύ«
#Bê?àȽI³8?Ðٛ¬I?À£ICžmò?¶*؆¬f'?æ=íj•äÈ?²—Œpø?ÂÞð[áJ?ªšŽewÂÉ?Ä)ZNL‹–?®
Ÿøû¡C?Ðä½üœÀ?´V£CÊ+É?â¤ÑàÕ9Ð?º	‹N¯?ã<ƒq—¦?©WD"æxÜMIXED4FGL J0810.0-0505?êuMÆ@-Ùh">À;EìSzÑWÀ<˜(=5ët@h
0ëp?úÉoŠÑ€?édÝÀ$5?á¢ÛA"¯¨?ù·$#Ë·#@N²OÈë¿ïüœ¾g.b?ïåèâ­â¿ãÊh8Î}§¿ØߕÜö–¿è$½"Zm4¿ïý'!« €UNASNone?ìé'q,-?Êi:eEmâ?f¼;±¼8?^Õ•¢Ý?·ý'˜lŸ›?Ê{úŠ¨ÃŒ?ï1ÛÜN
ï?MxÖÐ?vd¿"D?'`¶µôm?">kwQ®?—֐0isD?î_r:ýNl?š¾#.á?tÿËŘS?}vøËnV?¦<Uì|³?—ÐäF'¾?îCïp»©å?‡ë¦à1·?ƒ@˜*<—F?xÄýÿTsr?¦ðâæö‹æ?"㕽¡I?ìS\žïøT?È1Þ˜ûS?~zŽåø?w½ÏZNÄ?»}r(ˆ×¢?ÈZB&ý+ ?í¶³;£'?²üAöÞ2?'L¾þ
ºø? <ÿµŽ_?«÷ÅNø7i?®gœ0´^?íQ';7tÈ?£5´wE?†+ž)?'‰¢Ž´[
?²°°¬°¢ ?¡ãUšÿ.Ñ?ìгäÉmÈ?£Õä̾w.?/ù¢Ú¿6?ŒxÅ=Ö2#?·Ta£€ož?¢uÔýÏ¢`AGN4FGL J0811.0-5636?çÝù<cÖÀ(´Jb#á‡À:&Š®DÀ<öÉ™"@i¥ˆ€@«"}¨¢K?Õr4ÐÂ$Ó?Â'}mi?ôò†š¹T?þ{ZÚ6x?ïû":ŒÃÈ¿çÑ;&F»¦¿çM<>ɚ¿ÖôF£ÓYY¿ïÿJ˜ª†Q¿éyéÐé'ÿUNASNone?ï#¼{N‰?"á%ýÉ!¥?jV?Õh‰Ð?b*-t./{?špÀy°¯±?'ïíåÖq?ëø´}†?¾.OYl?~œq.¦:?†ìñÿcj?¾Y5ó¤Im?½è
Y¹ô?îvÒbôþ?–G´y¸¶g?"QÖbÕé¨?'§F)dh?£~d7v´ž?"9W&¼ß?íÎ!rãÄ­?‰Š³§ÜÂ?†z£dg–d?h¾²ðe'×?­?ù…¶?ˆYºeÔá'?íîs¾=½Ñ?¢ä'™I}ý?~VµQ,®º?tñ¿Q
rî?­Mís¶[?¡ä«Å#×?èC'«¶,?ÈèÄ.îû?‹_g
ÿw?"ÃυáAS?ÍAYÚðZ?È\CO'I?ìûAO‰2Í?¢ÅQ\r?'àýÉSwu?‰<Ólz{?³­¶«f;? ­ÕQ/ç\?êó_Ôãÿ?£@ü'¸¦?"´%¿ŠÍ'?"ÓÁÎA?Á»ûõ•?¢›ú\}ŒAGN4FGL J0813.1-5049¿ãù	Ž¤À"">À:W^!ôFŽÀ;¿jК¸@}ã ÷€@ü*EMçê?ɂâˆuÚÎ?ÃùGÿóë ?ùlsßË­@·Uê™?ï_‰ÓRù¿çt¸Œ£è¿æŠP†*Q¿ì	ÜW"KT¿Õ©ºy
2¿ïý3!jˆàUNASNone?åÏæŒÀÌ?Ãu¸‹C¸?ˆ¢*`Œ?€Û?2C>Ü?ӟŽ¯ÊwL?ÂÀ!~â+?æ,g¿?Ãòw]•Ä?ŠÄa$za?'1œ7â"'?ÒÖ:Á"VÜ?Þ"d²m?ê°‰Ó±v?ª2•ft¢@?•û^êøÛ?‡º=˜Ÿ›?Å^m¯Â?¨€ÊL·5-?ê3cP¡	?™ê+y~½?ˆ×ãs…ÈQ?qUŒÞz>?Ťô…gLY?™IËú4§?Ý©_'ë2?Ãò˜Áàé?–vvÇ
)Ê?Œø×Ìíõ?àÇ÷šµø?ÃÜj¤§?Ü4I…¨:?ɹj˜,åš?•ø.ÜI? )3™Ï8Q?á6,
?ÉIž{øì2?ãˆ-®Ð§?³ѲïéÎ?¦&-'˜kß?"ƒ¢ì?Ö*ßOŽç?²˜Wš¦¿?àÎz"}?«Ô°»²
Ó?Ÿ^¤Ò½¯?C«Gä<¢?Ümÿûfú?¬%HuMIXED4FGL J0815.5+6554?æÂ0wÓ@@'Ò^ÝÀ;Ýh1AÁkÀ=ûG3›8@!´u»îÙ?úÌ 4Ríä?Ñw~ý.?»À'׳…©?èÝAÄÆn@†újê°?ìDS­úпíđʘ?'¿È"ãw3=¿à·íu?¿ÄÓàR:µ¿Ü+Uc‰½.UNASNone?ï¤%Jˆ?…ãÚ9Ú²¸?=Ñ â¹u?5N±˜ç?†6®ˆ(?…ˆ
õ†?ïœÏ
áþ?†/Ẳ¨e?^\S*.Æ?dw!Cwq!?…-ÏjºH?'¼Ÿö-'ë?ïTevÁ?Š‰'b?`xÂ}vJ?kí¹<^Ø?š¤@"Mb?‰Kêeï0?ﴀ8°±Ê?ieØXe˜?>ÿ~é%±2?*ßÙôB}?çõí4zÌ?ic.ù¿«p?ï
l™Ó™?˜Ü*p"|N?P}é™'¦?J¬~=a?JŽ-O¥w?˜"Äλ4U?ï&Â웖–?›2m´Z?e1‰Ž)f?uœ
Å#]Å?˜q5 –{?˜Á!·¤‹T?î$³{(Q?˜‹Ë~,Ñ{?d/W¸£÷ù?p)Ýæyíê?¬{?M‰$ö?˜zçf{ì?îâϞõ_N?ŒYë—&ó?RÁŠÊw?Jþþ㺱O?¡<ùÁ³¥E?Œx|ÈBóAGN4FGL J0817.7-5258c¿ÑY+'LmÀ#:1…ýÀ:[6ÖUâ‹À;×ê¾O@8°.†{/@CºkáÐ?Úß©HcF ?ç/Xb—¤Í@Õ¸~a.ï@=Õø¬¤¿Õ#lì'dò¿Îv~6'·x¿ë–îÄnYz¿ê{åßBp=¿ïùV}»¿ãs_ÍSÛUNASNone!?ë•`BL"?¼ÒRá#q?¶l§¸µ …?¶ú˜l\ª?©Ð°Y•Ó?ªª?ô«›Ì?áÚä-š ?ʦ…vˆ-È?·'Oĉ=s?´©ÌĶ 2?ւFÔó?ÇÄm«‡¶K?èÝ<<'x|?°$é]®U?¹8¡/t"?§eEÌ_a?¿Þyù?¥nÅId'¿?æ<pøKçÆ?§YÜKb,…?Âb]oi;Ð?Ÿ›,âNMÈ?Ä«Þ¯g%?¡|Mk?çЧ^—ÿª?ĎLÉÝ.D?ÃuÓ¹?À¢bSd߆?ºÍàs?¸^Lܧ‹J?Ӝò'FŸT?Éþ¦d$º?ËwâsÁÝt?ŧYÃQ?Þ§Bő3?̧"«B[?ä¥jò4?µ½k´B¸?ÄP†h—÷Œ?°Ã*)dÌ_?ÉÍË>F&?¯šLqóV?ÕIªèeHs?²!ÆÍçüi?Ó$¦'ác?¸¦úȸµ?ב®"¦»k?·óð‡y÷âMIXED4FGL J0821.5-1436¿Þ.µybÜ2@(×bùÊ[ÙÀ;\>GckàÀ<ï/a›M@C×Æ%ß@*,©¬6T?ÔõD䋅?íâ_ !¸@Jùe²€?û@»×‡ÿ?ïà/€ KÐ?Ú,¢'¼†¿Ý¯»/¿ïáB‡N=?êŒäIÁ2¿ïôþ¯çÝUNASNone?êG.¬"$?½é[›(²H? N)p¿? P`̐ÀA?ÂÏŁo?ºÂ®È¢=$?éâ–^??ÈïOûã26?¯"Ú¢TQ‡?³†ë%¯:`?ÃÇÍ@¡?Å1¤
S?åû»ì¼ú?²ÅPžigA?Ç7ß=Ecj?¯æ=·öšß?ÀÙ4Páç3?¦'Ðr<Á?í`º;5ò<?¤–wZê?¡g û—e? k ƅF7?¨;OQðå?"òMÔÃ=?çE}ñ{
–?Ěiōà ?±^—©õõ?°WóRÈI?Ê:ûmbó¯?Á¯''ü¸?á.)qq?Ñï£g‰ã)?ÊLõ"¯…G?Ì~IÚȶ?Ð}2Y³>u?ˑ‡áO)£?áċÿÁÛq?¸mÖ1bi%?ÑÛÈ-*Ûv?·ìݞJ;4?Å6?¨ÈœÎ?©²~+F?åt‡_k†?ÃíÎÐ??ÂTï†
E©?Â
óѧÅ?ÇØòüGŸã?¶ƒ¡iÊAGN4FGL J0822.8-4207¿ámR_.ŸâÀ±ÕQ֌À:4®'xbèÀ;twlH(@!fø1ªr@ÆcÉÓô?Ç^«œ{vC¿ VQ›S-$?֜TŸi'@@X·ˆB[¿îø–^ü³?îqBÝöð¿Ýû
'ç¿¿çô¯¼пЈÊÿÃE¿Ø«úú݁PUNASNone3FGL J0823.3-4205c?æ;õêÓí?ÅÖ —Œ=?OÝjÛ˜W?C³WÂÂ$¦?Óx%Ã*"?ÅԀñé")?æ)PiW?̐ð÷€C?h'ê¥.Þõ?|trž?Ó}X@;?ÌKÀ)ȝµ?çÚ÷P¹¥?°J=R"B4?Š}HË1'?‡u³Î]¢q?ÎìR{DfY?¯šÌª«X?ìzºsÑ*?–)l~ç
?[»vúb{-?HTâØ-À©?»ÀdQÁÇ>?–ÉV[èo?Ýee1Tƒ1?Ç]QccÁ_?a"R…©?Uì:¸÷"?á<+œ8I?Ç][GEÜ%?ßR ª€­Ì?ΘúÁˆ?kËï
"Ò?†Æpé?à;#æþÀÿ?ÎG´«å?âTL0bÑå?¶±`56ýõ?–<ü×ùÈü?'`A·š†?Ùó—Ñ1OG?¶<Ɏ°°­?æ×Ï|Õh¨?®É/Ó: Ï?oGÁ]ùr'?eÚ úvÖ-?ÒтØÑ­?®ä¢ÑWŸDMIXED4FGL J0824.1-6004?~2áì©À)wùÖñýÀ;W†Ç.þÀ<ªZÉz1õ@!ÄÀ:Çý@üÑ\~†?Ü
ËD·j?ïÿ±eh@.Ý}ôøe@Jöô=ª¿á¼œ2Ñ
¤?åRqâpx
?·sëÇkd?îÙ²X­@@¿èù"»¼Q¿æ‡Œ+ÕqUNASNone?îT|Kªù=?²äÙmö?¤9<÷'q?²È#§œ^?‰ûù8¥2á?ƒ\D¥Ô–í?ì­Ð2\ô?Ǻ	ªèeH?°ÐXˆk»?Âu;Ê?¬tqég½H?¹ÒˆÁ:ü?í,e¸äÒ?¢;ôð#áS?¡åÿ/ÂÝ­?™L-kx=?«S°f£,?š>zò·?ë8C#ïÞ?±²ÌÃÙe?¸|Vžºn?°<´kuþ?¬rÕsñN? ¼~̾Óô?ëcÈÿ…(?Ä{˜ŠX'?¾Ÿ¹ah®H?ÄÇ×Ð6
Ù?™ ÁZl¡Ù?—™5F?è3ÕA\ãþ?ѱ™¦"Ä?ÂÔ¡@Š'?ÍUãÓ4×?¸¹4°ßüí?«)‡‡¯?ì'Nm?¦xe{º?¥Ümmêè?.ÑÝToÉ?³×X芩£? áày4ÆÇ?àõ… Ctý?˧{÷ßå?Õ\øȗøž?Ï3œ
s\ª?ÁoùíÂ:Î?ºèÊK_œAGN4FGL J0825.6-5216c¿Èä9RNÀ oŽ\NµpÀ9¿MÈ	ïmÀ;Š
öÔT@/A:2@'âƒw?Êy@ˆ±>ý?Ó¶h\_ÒN@Ç>Ê€Â?ö#õ¶6ˆ?à*ڟg¿ß]e¡DˆÆ¿ê¾'¢O¥¿ï'Iž¯ƒ?«ØSœ<ê ¿ï•Û¿-ý¿UNASNone$?ä2n3(:K?Çç(t#¤†?•4é·ç?©•˜þ;4?ÖAPJxÒ­?Ç1Už©4(?æÒÁ[)œ\?ŏ™ù¡þ?•­å5dÁ?˜/ê±í¬?Ðÿ«Œ5Wü?ÄG]cÕµ?å-¤•
#?°É^ž¿ö?±¦¿MZQ? ŒëDãÞ?Ñ;$Ç?®ÑwÈ·´û?é¼|"˜äÆ?ªªq«"vÉ?š:Ìæ•NE?Œˆçtâ¸Ä?ÅƵÚJ—\?¨c¦ïG¿ë?Þr5w08,?ÉZêQ
?§'z­™vv?ªD»ëá¸?ޛ›3o¥?É*<"…Þ?Û¬Q-U^è?Î9$ŠýŽ?¯˜dmkÈ?µxJð›?à0Q"v;_?ÍœŠËܞ?ß´ˆ2i	?³¿
2+ô?À‰?ö ih?­aªçݐ?ب«{ª…?²ì®Ôê'§?àâßmä4?º£-Î福?±ÉºRœ'
?¨""cM"
?ÙÇҏâê#?¹ÜJ¿ÒúuMIXED4FGL J0826.0-0157?ï§'§
öc@3öˆœTÀ:­`#VF^À<u°ç"øp@ÜÞ'h#Ö@DÙMä?Åßïÿ¬Èö?³íDfŒQ?í./ˆƒÇ @ª6+‡m?ïýI1¢9¿ç>¨Fۆ¤¿áüHKá¿æøÒpXƒ¿ãÆôµ¿ïÿÓ?,» UNASNone3FGL J0825.4-0213?ïÆÑ[ãç­?oeÁ˜E?Hš
¹'ÝÅ?GCklÕm­?y"Ðòž0?m	óªwYs?ïȓšy?wÈšBi?P"Vcu?VÛì2!?w®¸‹‰wï?s÷(б§?ï|)¥Q?{lqöÅø%?cKŽ´[^?bª
ÄkW?Œ"²øßQ?xðÈVÿÁÆ?ï«;'4?]§_¯®Õ?bmÝ"b?Cy0¶¤+?€ ùë'S?ZAA)E=?ïsfd8
ã?"oY¸(^?Ylt«w4c?R‰qÙæ(§?øØQ6ê¨?ƒË ¯¼ág?ïi"Æ,/ð?Œ*˜‹ÐÎÒ?aÏ%üß$?išÉšhK™?"£{é²?‰l%Fâ?îñ—Š©De?Œ
@Ô90V?p÷Æîäì(?kӓ&ïA?ñ…òP?‰Ø}È*?ï7±$Ù1?z0ykcÔ?wdO8¹O?`ƒh¯ÀÇ?˜öÛP?w½!ïv~AGN4FGL J0826.1-5053¿îÔ6}jÀŠòQÁ"´À9ÝË£!hÀ;©Ââæ@ž3×Ú@I6'sg?Ä!Z˜§×?АA–£E@
Ä.bT@kK
¶!¿äïv_Ø­¬¿æðÉ+WœŸ¿Þïeþâs¨¿âŒèæÞÆÊ¿ïÿž ßt¿è««Ÿ«yUNASNone3FGL J0826.3-5056?à¹ÀÜöÞ? H!#] ?®—ê‹Xù?¡_¥1FVÎ?ÚºÃ-oW"?Á¢h"DôY?ã+æò#.¿?ÃÖ\B¡Z?¢y¶ádD´?wú‹Âƒ'?×Xû?ë?¬•bc‰?åjKª<Bë?°ÀØÒÞ?¸ÍkÁ	Ä&?¢Í°ôm?Íðweù??«®jâÒ¼?åèYÞÌ1O?¥G/êSpj?¥ÊäúÊ4?ƒŽ;@?¯œ?Ñuï¿Úº»?¤¯Ù·*Ÿ?ÐQl˜ž`Â?½vjž"¬?»Ü(àIz?°0†Rˆ?ä[ė?0?ÀþÝ‡§v?Ö$r6d|=?Çx/mNk?®ó.[FÛ?°ðښ¬k?âþ"%Ëä?È
tâó?Û2ѽ¼'}?³~fØ9ù?Ä ¤ÿíû5?¨³»Á¨$¤?Ú|ÛÂLÚé?²,îN?Û6Z漞=?°ĐúIï?²ïµá_D?š2ÎxVP?àÛÐ1Š?°÷Ê éè8MIXED4FGL J0827.0-4111c¿Ð0îáZ߆¿úköÉ™"À:"'‡V ÷À;‰Õ¤â¢ø@!«t0Ô^<@dïmâ?Î`R»Ž¶è¿ŠÄ©Šô¯?°:³ží/]@+áìõ?ã@JÞJ£'¿ÛçÚDY¡1¿é°Úþ¾·¿áírÊ!÷¢¿ÂN9žÝ%`¿ß¨bÑÜVUNASNone ?؝¶"«…?ĉ‡ï‰K?a<ï‹?V}Öo-á?ãŸçÿƒ-q?Ĕ
"ê™x?Ô!ûk#m ?ÍýÇt%õ;?‡5ÙP?'—»*ài½?咩v,Ç?Ít'Ç"Ç^?âÍ
5›?³æ'Óµ?ê+'Û™?…V÷ü"?ÙWI:åæ?²×î{¦È?èû9µÐ©?¤Í~Bcv?cøçYŠ.?Rý'™?ËÃÓ|ÇÚR?¤Ñ_A¶8?Êb¹aúµ­?À÷€]1?k]â­Š1?fúh9Åá†?éKóÅb?ÁéS|e?ÊÖsc=Ö¿?Äã usþ?zB[`?ŽË«ÿ<?éX¢êŒb?Ä´aƒ ½?ÕªïüÁuð?²1k%ŸF?œß/kv?Gòä·ÅÂ?äJIv_ò?²|CøqN?Ý`–†?´*6'öè?vF7sëÿR?poÌ©ÙÞ#?á#(Ž"'Ù?´JÌì.ÝMIXED4FGL J0827.6-0059?å~—eóS@4Å2¤—ú]À;lWÛÀ<™ã½ª@ 
ããê¡?üe2.?ÓÓMÅZ½'?Éۥá|?õªŽI@Öې	"?ïýÐ_ÿD¿ß:Ç|*óÊ¿æAIvk—(?¯Kì_ÁW¿çIéXÎG¿èsHÎ÷ŸUNASNone?ïãü/՟s?o>âøâò*?Gx†Æ=r?lt49M?f%Ë.]‹?Uí&žF_?ïÓڑË2Þ?q™tڗ@œ?GÚÁYÐéô?RÃÊO
?s^÷ø@¹?m"×Ø?ïqñð·?)Á²ž?jËÏß?Wç?r4èÖ÷Õ°?Œé˜gT?{‹£ô?ï‹û#ªÝ—?h}´"<Y?^:BI<°?EdQ"8Ì?‰9îÌ'•?gejÔé]ž?ïÒþ§Kš?ií_#±÷é?M!نQí?T·Ð#¶îà?sUE–1?eʱgŠ3?ïƒyݚ-?ˆË7e5Ӑ?[±'?h´"&s?‹«e¼m÷?…¯¯ðƒ?ï	é«T×ô?‰t1›§'‹?ul¥]ݬÊ?xo5Ca?™g¡=Á›Z?…Ååˆø	?îÒµJ?"\#†0Êè?o*ìØÒßÌ?c.¿7¹â? ëÅ×ØG?ƒ›tLoz¥AGN4FGL J0828.4-4444?Âù^6}PÊÀ ¸Ý+¿¡À:|ÀØ£À;Ï™¹z
@ ÔÊCX@é@&?Ïø‰ÿr¼`?ë:I½cMW@:ð
­@]"N+1¿è¦î·`-¿íù䒼/Ç? ¼«³¿Ý±cºº|¿í½tŸå
5¿ïÿþÞ÷UNASNone?´i¢ŒM?°·8Oá?×üÐERD›?ÄúF$Ö?átsúp‰?Å«Á­gŠ[?ÁM
+<?½KòöñÓ0?ÏSì›@°?ãÆÛ¾yš?ã×ü?În…?ÃÒCh&I?ÐCzˆÝ3Í?¯sïk&Lm?×¾¤t­À²?³,píu[?×ýá‡ì??³lUå¸÷›?ËàMp~ËÁ?¥Çͳ¢eb?Örìláf?³˜ƒöÃa?Üf[S¸º?±ïÀH®:S?¢+½V¹Õa? ½oyÄï?׫i;¥??Ç4°‰¨¾X?ã{õÍT»?DZÕe!ÂÈ?¥ß46"¤?«Zàxà˜Z?ÑjƒªL¢Î?ÉUØ?­Ñ?åìÊçwüo?Ⱥ+An¬¨?Âú8W¬²?¨‰íJ¸äL?Ü9	HJ"ï?¸˜´	ýòÄ?ÚIꉕ¸?¸e[órˆF?¯dzPÍÉ?˜0µ-šà?Ü;š'u?½z@kˆ—Ç?ß×Öôђ?¼…	OñMIXED4FGL J0829.3+3729¿ã¥ö!vÿ@A`mqóbcÀ:Œ»NŸ À<xÉÓI@§6õŠ†+@0ïVd£?Çá£Þìßè?ѐíBäE@Mjßqêÿ@ì؜¹´—?ëG™ò"í¿å¥Ì­ÃJ¿é¥ß™±¿îå7&ݺ[¿ïµ6þ™Îs¿àЏ¥UNASNone?ïf"Þ8e?Œó¢!ôµ?rö'셈@?l
€do?Œü4"=V{?‰ΐWŒÀ?ìQà(ãè·?´e‹Nl
‰?°r¦ÉÂ|?®¢Ï¢dûJ?©ü¯Û¨ÇZ? RUuÀ[?í˜&õ¸({?ž‹NN·‰?˜í2P'È"?ô41õk?ª÷{X-A?—¿P
ÏÿÂ?ì²[ºï]N?'KF¾+?°ƒçŽÿ2?±´˜Œ?£ÒvDá¸?~ød"–?î—<×E;?¡þ&qd÷?†G£ž#mÎ?€añ"È? úU8oç? >Ž"?æÊR¸ÎVÿ?ų÷ˆz@?ÅT:º1?Â|†®…d?¿?ÅgÓ¤?²<YÑÇLI?ë3…JØý?ªU
ðà,š?¦îç|AF?˜"HÇr"}?ºìd>Ôt?¥»˜Šåq•?æ¡Þô ?ª`±?ÆïÆò©f?©ímùz!?½åí§…7?šV"(Ä:AGN4FGL J0832.2-4322c¿àáµó8À<œƒXåtÀ9˜4¦Ð¹ÁÀ:‡l¸K@ ½[8á@½·B÷ÌU?ÊV/wˆ¿g$b­@¸?¹í•W?@YBkàMÞ?ïü÷™Ã
¿èË÷º·!¿ê…ñxô¿å MÈ௿àùã»üšñ¿è!,À¨QBUNASNone3FGL J0832.8-4321$?Ì"•+JÜ?Â˹Ë×ô?p†ù?§mW";Ý}?è\³NqQ?ÑýF.?Ûâˆx?ËÖÉ@âY?‹û¤jÏ?•%εtx?á¢wՊǫ?Ë+ä
ÊÝ£?ؔ½'¾?´gçtÒ?­‡=¤åÍÜ?ž%3ÞWMj?áÝ-d‰Ž×?´8,jàI?Õ²¦Â](?°>îÏÂOº?tVA#b?Yñšøc?äþ@¹•?°EØ[´!S?¶>뚏°.?³ÃÓÍôŸ?Š£µV'{l?'$+rüù?ì͓·ŠùÌ?´¶˜kóÎ?ÎQ³©Á]?ÃúfKl´?…Ë Bœ?"ŽÞž"&Ô?èéDQ¿?øòùý§?ÌRœZG?­Ç©Rmaã?¬K{%%®"?˜ÅÒT¦²?ç4³¦é–æ?¯Û!*EnŒ?¿‹lB"ò?¦$"ùâJ?zVG{9ë2?i28þv'†?ëÙåî  ä?¦PÍSّ™OTHER4FGL J0833.3-4342c¿Ä¯áQ
¬À—)|Ñ÷À92\ça£‰À:T@ ¤		>@Móùa€N?âÝÄ6%Uû?Ôñ†U7	?ò&˜Ö%;#@í‹k®yÐ?íYÌúïõÇ¿éPCD"nÀ¿é$ó¿ÕÃk¿ß.^b6¿ëÏ*à~Zy¿æ‹¿m"¬UNASNone ?±ËÖÿ;ñ?³ fèl?}3Œs½#N?€(®ùëÒk?íŒ
K©?³šWcŽü¥?ÞÌèQž¿Z?˙ÊÞX?‰Û¼¤—–¸?"9èl'o?à2ä¬h?Êë2U41W?Ùt¹å-Z›?³ÊŽþR?ÀœþN¶,³?©T©øh?Þ<Æów?³yÃK<ëù?Ñ;÷6´«?³#¨Oèf?pÝ1(kÓ?e&õýß?ç@J¶c?³mâ"ñt?¢±zn­ž?§™ßbC»?qZ¾¨tæJ?wÄ6ó~‰À?î²2Ûۙª?¨"¹¾y¹/?Ñ]º!ñ¹¹?Ä䌑É@¦?‡ã©0¦é?˜ã3‡*?æñ"J'ã¨?Čä'±?×O–k;ã?´'èdÌ?¾ã¿(Z£K?©#¾ ?à"àO¿
¥?µIYkA?À:¥¶Ä‰?¬m¶Šíº?gkžN'1õ?n#dþAAô?ëÚxMt?¬vÃ
§OTHER4FGL J0834.9-4612?ìÞYHÌÀ¯"9櫛À9G6v¾À:¯"½i'@ &K¿ÆÿÙ@q̾Šë?Ëjß\qp?¬)œÜo,3?å¡ä¶Î^?þö-pülx?í4T€ŠÔۿ뮛‰]â3¿êj •6^¿á?&¼,k™¿ëPݾ¿¿â†œ1#Ž{UNASNone?¦ª	qvmx?¡+\2–x?†'ùØ?†ÝŠ–8¿y?î;"Å»Ð?£ê~u3°?߅•PM?Ȃã}@?"`/%îM?™Ý2è¸û/?ß4}xÚ9û?ǑŽøè#?Ê¡9OpÅT?¬éK»BËR?´Ü®ÆkM›?¢\Pü±fÌ?æ¼ÓVdø?°~]|R£ö?¸M·€ÐÃÿ?;Ô]²/?B!¼Ö?t7´2ØÉ?ìy@ŸÇý?Ÿ:§—m¡?Ÿ|ÌÓ?œ½0#h¢Ç?}¦Sÿ@?|naþfé"?îͯÜY»;? ~ô
)?Ë÷šù".?Ô3 Ëý?ž<Â(.s?¨u¹˜!%h?è30{jQ?Ä4@*€?ÓÏåìï?©	ü¨éŠ÷?°µãÔÏ?ž´'ò¥1O?ékê´¿:?­u¼VÉ?˜?é"ïëÔ³?‹Ìqi?'øuˆrsÉ?"ÅÓö?î€ï¬JÌ,?'c("{MIXED4FGL J0836.0-5458?ÊÌÂ×¼¦À!	(¿;ê'À:SEùßTÀ;æÂW(@A&œÍ@ˆ!¢7?˘iñŽM?Áøü–'O?ô½áâއ	@Ûr±Î?ä•qì¬f%¿äègÝßÄ¡¿ë¢_:øú¿ã
+Í
dm¿èÕøÅy¿æ¤O QC¿UNASNone?ídzw*?ª2qÏø'?"gK*ƒ0Ö?€jäêÉO?´œØýØi€?¨6ÊöÁm?èµ	UOxõ?À=
š¥æ¸?€êŠI…à?'"™=l]?Ì2òÄi?¿¥ê,PY?ëÝɇÚ?¢˜ïÓîò?"ÓÃï«	‰?‡¢ãD]}	?¼"¹ Gž? Áîëà¦?íߺÊ/¨S?›`ãØ?‡#ÁtUǛ?aZ¸=_»3?¬;cËïè?éòj44?çül+ï"o?½Ù!w|—?ŸÌ÷õ,'ä?—²LIØܾ?Ì°Råød?»"|""€®?á–0Hû¥?È0.È?'="¦ŽÌ@?›Îh]€q|?Û¿Æ#»F?ǽZ`k%?åÎü];Íê?°".'÷`?¨Ó'°à7?—3´QD¯÷?ÑG¥MÅ?®·`úy?éҵݥ•¯?›Ëت'f? «rÌ/«Û?h%žÄ'—?ĊKÕ¸Ñ?™ ó°/jùAGN4FGL J0836.6-6036?ïÒÓ:éÐÀ'õûmÊÀ;ĘÚÀ=Q΁ز´@ÙÁ®‹™&@'$·omv?Ùè—ä7Íw?ïÿºà¼ô@zœ™(Z'?ó¶Yh|O?ï¬;ݦ¹¾¿ÑÏ£@âH_¿Æº–ê<Ê6¿Ù£C;"¿ëØMú^Ö¿ïøg_µ0UNASNone?æ½J
1©"?Ç*QôO®Ð?ÀcG3VÐ?À;†(^Õ?ħ£âÙæ?¿•‡rƒß?Ïw:Ÿ
Kî?ÊÎûêáN©?ÒÎ?gÇ˜?ʇOEž«ã?Ýv#Iþs/?É\+b?çÊ7ÁQ?±óì=®ËÖ?¼×¸åJƒ?¦0%‰<ÚE?ōLŠ®Uz?«8öÒÀé?ÒÃJHÅä?²F_zíC?ä"CòÚ?³ 'øŽÉ;?°÷¾¬O^?Ÿð‰çá*q?ä"ªc?ʦYêñ¿º?Æ_ jj?ÁÁ)\8?ÉVÍ_LtU?Ãôû£G?½œ·h.	?œ03	ÓÐ?؍?Š҆?АµŽÏD?àÉNyEø?Ï¡;"B×?ãÜF…~S?µ>8+tàÃ?ÁÓ£Ò­?©¾—±¶;©?λBÛ5µ?±œÂY[…?·¨—xØ?§*'Á6€@?éÓ®!ÆN?¶Ï';¨×ã?¹¹÷{)ʇ?°ženë°MIXED4FGL J0836.8-4638?ᓋOûôÀ»Ä?_'À9m.Y°À:°ËJì\@êv¹DÚ¥@<G䛬?É@tú¨Ó?²µÔ¶a{?硅‹Å›€@ÑQž?ïò÷ÙÀÑ¿í
°'z˜M¿åÆ ©T¿å³Æ)ñk¿æÁqN÷´Ø¿ïÿÊ»z"òUNASNone?Öo3R?Æoç³F؛?€ÔÃË£*]?zQ}ßF|‡?ä»uiŽŽú?Æ¢;èqw?ãxߚ"Ñ?ń:õ°'?ƒ¦ÂôÊ(k?ŠvnNð±Œ?Øq
²i&é?Äöv/mg?àA§?I—?¶	·Íïß?ª9Áq|?œËcrŽj?Û¢õyz{'?µB×£Oí?Þ«µðoó?­Vƒi[­?ƒÚ÷Mx©?eYÈ®½¾?à[Çû#D?­N'¢µŒ?ÄzóW6Xé?½yá|˜h?z´³µ&xr?w䠛›óU?ê«ÙÂÔ{m?¾1DöÕ	?Öi!Æh?ÅáØ·Mñ?†õ¥˜‡I+?›ÈÖ`-îú?äo˜†Ê	#?ŊÐ.'J×?×Ô|i2´?µ‰Í²Þ‹§?¨<,¾ë[Û?—ÀBN#çu?â'þÿ"¸H?µ£/l®ä?ËÃPú\?«R†k±­K?-	i{?wS¶Ý‹"®?è›:÷€];?«…Ù²4øMIXED4FGL J0837.8-4048c¿ím@#ì'?ˀ.¤SAÀ9M1áú[À:µƒßóðþ@~;Å(@6¦Bˆ?Ç×Ñ7À‹¡?Æ$£ç"@߂±ö‡±?ë`s/¢"û?ïýAԋ³¿äè]_V¨¿çæ끘Æá¿ësP$¿ð?ïÄT=nöXUNASNone3FGL J0838.9-4056c(?Þ)Üγ½î?ÓY´öí2?­ã¾2_Œ?ÄÂ܀km?Þ²øª!?ÒùRa:œ?Ò²7jzr7?Ëùf=¡¡%?³š-=¯U?±w>¹+ã¼?ä3ž¦ÚÛê?Êô-›¼?×<ÇQôЈ?² «ܚ¿?¿Í8ºSû?¨ŒM/ý?àgõ?»4}?³—¯Ü"o?ÀË=Jä)á?¦dìló©?¹Ó°pŸš?Ÿ»ÅñïϏ?蒺ŸE!•?°h7Ž‡y?Ü
Œ…‰í?ÒÞ–üu?£ÜÕ­Dg?µ-"©6?à³8l‹¢?Òíqñ=?ºªÔ_a(?ÁÜv'i?´µxó0ä¤?µðÁ\gp?êö^÷F?Ä(Ç}
J?Ò偅aå^?±f‡®Á'3?À#ˆtœùº?¨‹ÝJFÀÇ?â"] 'Îâ?³jjM?¤2.0­†?"Y÷…A¥?¼J}I#Vê?©,(zc§?ë3súj?®•ß:ÞYMIXED4FGL J0838.4-3952¿Ýø¡ª'ÃÅ?ë»'ˆÛuÀ9yo/bÄÀ:Ó¥á¦x¥@˜é6ºÒ#@ÿ^Ö?ۺϟ:~?ãqbx›Q@jl»=¥@"©ë¡ND¿àq¶ùê¿Ü&n¿%oP¿ë²ÑCT§¿ìÕwácà¿ïûJ>³‡?ïë/=Û,âUNASNone?Ùô›ž]?È[Uë]ËQ?Ã¥"?V=`?¾þÉ|w±?Ü8Óȶßó?ÉÌ% ?×]û)<Ët?ÐnMÕ9È?µ†9Þéœ÷?³ô:&Ü?á ;/'%?ϲZ<®Ôa?ÝLbìOý?¶æšwÔ¼Ÿ?¾E󔷲‰?¦+TÌÈá?Û"!åÃ`?¶4ÅWÙ?ÒåF?®M´Ê¿¯Â?»$XÏÏá?ž5q™"æ?ã%bÿÃ?°YPa€ô=?ҎH·B»«?ÄíÆ3î‰?ÅL|ýŒ?Á)gDmÿ?áeԅ[‡?ËïïÖUü?Å&Îljþ?Å~΃†?ÄjêRCÅ?Äà1Oû?å›Æ"ˆïŽ?Ë¡¾³?Ғ×~褀?´KçSôX?ÂY²)nŸ?«®¸šÓºÚ?â '¶0à?¸›)8H÷?²°MuŠ¸Ú?›& YŠâ?¿wß'ËԈ?¯¨´H)a?éºúl9±t?±!"éû]ŽMIXED4FGL J0838.5+4013?æ|÷ȁ—"@Bt# –x}À;žU9xÃÀ<Ò³‰.èK@"Ztâ*,#?ûA*ØÞ©?ÆʙÁ²'d¿—…ã{²Jb?Òr>¡ÑL?òh_ōh^¿ïÿÿ" 5•?ïÿnªØ†>¿«2Zp8ø¿åÍ}å¿ØÊE¾¦ƒ?ѳžþ]h'UNASNone?ï.¤§®t?¡ßm"îž?N¿·Üié¤?Lõ°ÿQÌ?™5mQ‡Ê?¡¿«ùƒê$?ïbGûÂ-·?"·™ÌÔ¶N?p@.xIKþ?|*1ÌÁt?MéÙ'B?Þ€¤6Gé?îZ~zž¢?™žìyA]¹?zP7@67?€{;œ ¥?§r¤?˜™u}Æ?íìüåï2¨?'ô€†R]ÿ?ƒ»S‰2`?r–ý]*?¬A\»ž¥h?'ëʾ#?ïÔÜ÷Î?¡£ûôâÓe?aÜ¢ÇÜsA?^X~ý"3h?Ãñ©Æ?¡€5Ê­¼?î]žá×öÌ?§Ú¹*'ÿ?`‹ÓÅÔ?‹ÿý­"—9?¥ÎüsûÈ?¤iÜFû-?íÇ®LP‡ú?œ˜''l?€.]ó:Ÿ?f»vâ?¯}¡îÞ¸?š¸I±Dž$?êAx"1c¶?«ÁãúA?"z´ò Õ?%Z%½G?ÄjÝ·‰LM?¬f¤M€AGN4FGL J0838.8-4552c?ê­TƒÝ<(À©Ðé'ÿqÀ9]U÷ƒY¼À:2`Nq@ o]µ<ã5@—¿|'1ž?ß'kŸ
qÉ?ìÃ-±@`Æu(@qÕÛ>U¿Ôºªö¹/a?ê_ä¡Õ¨>¿êvåں̿ãá"ßþع¿èEÓI¿ïÿÙÔóüUNASNone0?rI1&߁÷?sŸÖoôó?|])2÷¡©?—°~—Èy¥?Kqm?˜ÙõÕ.Æ?ÎætæY?Æo~³9RÝ?²8ìõU?³
Y¿Ü?åÿB#w9¯?Åää'K?зè÷GA*?°VI^~÷"?ÅE¬P€?­^Ô/Á2?âR§`ñKK?²·ÆCZm–?§"€Þ6?Žñb-q¨9?¬'‡ãb2?œtK¿6°B?콯ŒäÄ)?¢Þw4¸ñ?pðŠÔû?uï{Ԍ?÷2,Ÿ.¨?ÊðK#ŒD?ï–C3ä?")Bqÿ¶?µì3ãdòQ?¶|!öù/Ò?¼¶ß$¾%?¿댫t?éÂb§®Éñ?Á/UœÙXæ?ÇØ"­» ?©¡À¦+u?ÇzWJ:?®jƒe&®?ä+Wb/	?±ÝÍQm.?Œæ‹'7ã?|»Í‹b™?¬Hæ[µÊ?¥«Døéœx?íÇ×lZh¤?¦h—oÓ
OTHER4FGL J0838.9-2502¿íÀfÔd4¢@#¿¸jßÀ:ˆ[3,}7À<GĐ¾(Å@æ)ÊÔ¥@ºñ¾Ýa?ÒϏìTR?Ùz®ƒ?ýçdã¯ga?õL®Cõ£0?ïøbaô瞿àpLÎå«Á¿éí{˜ý'g¿è%LÀ¢ó¿ì'¬Óª7?ÖÅ|vs#äUNASNone?ä¢#:}?͍*ú™R'?˜ŽÈÄÐ5)?˜ÇOkj_¯?Õ2ÌþB]?ÍÖÎ@ÈМ?åuX°xÍ?ÉU26ˆþ?¼;ô[Ü?·‹a5á,?Ì¢÷LŽ_?Ä
B2ÕjU?ê9q^< ?§™á6=1?«½`c¼?™Õ¬ñðZ·?ÀXöâÜù?£³2X(?å…£Ì'?©$¿püi?ɵZ.8'[?£mý=ë¹p?Â4@q¬? w'Ù¾Áª?àì¨HDMž?ǂý3O–I?¦—°÷‰Wæ?¢oae4]?ÛS¹PFH?ÇצÄ5¶?Õ»N%õ*?ι²³ñ߁?Ð̶ßG=?É!ÏjƒMõ?ÙxHҒð™?Ì>@Ï~?æ¯Ð~ÌÓr?®ÊüÃ)?µ=1䩍X? ½T&–ï?Ê¢%wëŽ?©\ɜ¦Z?Òq&æ@3?®œm'\ž?ÙÒã]™†?¹=@³ÔwI?Ó¼zmÀ‰?µÖ
Œ\NMIXED4FGL J0839.1-4613c?ãÚ¾§ðõKÀ>‰¨‹À9q ٔ[lÀ:ªi³øÀq@ ¤ù9@FE^¯?Í'ØŠE>?ËHoÛZ.J?öñ§ãxu?ùSj…ÚÊç¿îcϝ·‹r¿ì "@º?î፞¹"¿æäW}•W¿æãyÌz¿êøsCÄ{UNASNone3FGL J0838.1-4615$?µ¥vG-º?¯¬d&º?wÙïÝ?ƒxðí4?íuKY?°‡UÞ|ú?ۚÝu€N‰?É¡¼¼d?•æŒŽ¾o?˜ù,"ËßÆ?áƒ\àøö?É	¾0°?ҝ£ù]¾;?°5ûƃ?¿/Ð8xR³?ªoËߤÜ<?âË3üBŒ?²œvQÚ¬ù?ÁHàñKÕ?§ÑX™;~E?'¾GÑ?…ÉéUŠK?ë%Ç-Œ¼M?©Ó¶§Å¡ø?§¶Ûå<±ì?¢dó©Z?A[Å5š?€N‡ÙoöÈ?î?ÄÃó?¤"çR;	Œ?ʪ†9H(Á?Ò?ÙÅêÂ?šWáÔ õ'?¢—Ÿ&Gþ¡?肟cvá£?Ãs¤<ŠÊÊ?Ƶõ¢¦U?§ÍŽ|z¼ï?¿}öv¥‰ù?«ôúÕ~	6?æbü3Â¥,?±€1;&ë©?­¨0Õó­…?že0ËÒ?'	âg±?"ÞBÛ!?í-ÝÞÂî?¢"º:û‰OTHER4FGL J0840.3-4544?éÒ¹Ë4¾›Àp²˜À:±èkŽÄTÀ;ºB<»r1@#'½@è¨u?ý(&¶Â?É£{æÖ¿—çÁ<BGð?Ñ3¢÷¼:@ŠF~¾w¿Û¢<€cé¿ïùÔØ4	?ïgÖs>»ý¿àÔ&~ïʿ嘑AƒÍ¿¥µna\'PUNASNone?èõí
7š?À»Ÿ†v?VP¶yy?H³nvû¦?ÏWˆE;üä?ÀyÌcŠ,Ù?Õ;»®Ï"?Ю4BŸ.P?ZEÖÙØ?‹sZ
z'È?å¹XÉN?ЃxfTY?ç͂:"Šó?°s=fR?‹ó"?"mãŽ'q?϶åÚºÌ?¯}åÊNâ?åÃ1æ¤\?°ìÒA¼ôú?r[äêgGÑ?g¯¡x?Ô0Tám:?°õ55Ô¾­?âzVD§œ3?ē™Àäj?e.TéÁ>?[ÓPÌڏ\?ÚàöÍÌç?ĐO˜ïz¢?Ðé¨	ôËn?ɞI¦+@?un‹s~"?ˆêߺ?ç`Nåmû?ɉó'ÝÚ*?âOæÊÍ?´åó§f'¯?–iô½ ¶?Œ0´ö
Û,?Ùú$涥;?´—Bº˜Jm?Ù@é€{?¹0îàGÿ?}"õŽe¥?`HZ?ã%° 
:Û?¹R‡šë2¦MIXED4FGL J0840.6-3130¿×›Ø)_å@3Ð9h×ZÀ;Ué'9YÀ<ׁ›v¬@'1È$@ü.Êî¦?ÖÜAÿÿª?íøЁZ@ñ¯:ÎÄ@
$ùS¿ïþÊá:B?ïXÛch…?ݼ"C¿‹¿èÐMUhÇ¿ïÿôÕ÷?îb¿è¸¼UNASNone?ß×_²íþv?ã–'¯H?É
§yg[??¼‡z™_s>?ӡ̐^Së?À‹ E
û?֟²¿Òµ¼?Ë%ªF?Ò~q¨—kõ?Ňâº^3?Öáۗ•ÞN?Ɗ01Ãhí?ã,TUÜoF?³‰–ÙU.K?ÊYxïLuò?¯ÈY¡a-$?Èõ5¹AÌö?©üÎóY?ç †N
?®ìÇ÷¢yÂ?ʁ´¢«Þb?­O®ä»s?²ï'†–6Ø?™™¡lÅÒ½?Õ4þr'Ý?Á²:Ø̓?Í^9#ë *?ÀlÅâ3"?ÜäíªèÌ?ÃÛ¹›Ò?ÈÜbxèk†?DZÞ^ð{S?ÙÈŠÄл?ÍYւzŒ?ÙÉÈ8Æù'?̼˜ÞCþÄ?Ùå<RÊ/í?¶7r\¦ºŽ?ÔÖ&òKü?¸´j†TÅ	?ÑDœ¹Öó9?±GÇ>kZ?Û\"''?¸Ð_}â?Ù.ÑudAY?»4RSE2 ?Æé4ÞY?±UŽçr—MIXED4FGL J0844.1-4330?èr-dÅ°¿àíQÂjs;À9Zox]߯À:š‡–ü@Ãay@ y½[?Â?ÎàÀʊþ?ڂZbÌþÌ@
RÈ>Ȓ«?ûæ"KÑ吿ºÐûۃ¿ëéz'}¿ãÌôÀ0Ý¿í:­³N¡¿ïÿ~Ù#ó¿ïûR¼ev|UNASNone1FGL J0845.5-4327c?À%Þ:LEî?¶´2V0è?³ÓÎ5zÆ?­ù%0íÝ?é|ªxö?¾o^ƒTD?Ê`@Ÿ#éŒ?ÂO$C4?´"JoŒÁ?¬='$r€?æՆ–ÿص?ÁFêï'a¬?ÏÜü1‹µ£?±rÌ|û?À3tcK¡6?¦ÄßX¾ÿ?ãûãÚÊ*J?²¬Íeç?´ªcºfM$?•Í¨öÊE?¹.Øü‹f?™
Îæ%»?êDØi/ß?£·›W÷È*?¬Çå©´ç?¤ÕӔc»?±%ü/Ò/×?«sp{?ìûƛ—?³ôÕØ`À?±#˜Ð4Ð?²ñl\C—?¶'5A6s?²ü¨èÙ:?êüæg
ç?¸6´™þ'ø?ÁØ#?þ¦A?¥§æ8ƒª?¾ba½÷W?¥Í"æ´Õ?罪ø^…?¯÷Ë÷6n+?˜x)rÅ8?'°	¤lÒ?»3Æßî?¤ܼú‰Ù?ëÙÅØù?¥üŽG¶4öOTHER4FGL J0844.2-4554c?×tö")¿ÿùyÔttÀ9N:¶~­À:³>Áï-@"#êÀӚ@
KáQ?ÏFªâ?уZ{w?ý«·ùÖñ?þQvg]?îyÞon¿å<5œ}z¿æe墆¨%¿çœ&;Ó륿åéÀ°3å¿ïÿî,˜å?UNASNone3FGL J0843.1-4546,?¼}ç¡åB?°\>]ò?‹PIMCG?ƒ»xY‰?ìçƒ(á?±¢eÐQW/?Ùí80⺺?Æ4K®v—Ù?šÛ'ès'?™D2C'?â2‡X=G£?ňå®èWº?ÕÔÇˎ½?²šÝøuÓ?·EbY©y?¢Kùsa/?âô˜	³?²ü€&ëw?Ç pºõC?¡¸ïN›³>?¥‹úmƌ?';u¤°Ã?èæû·@&?£B?œvc?µ'<÷	êÃ?«jq,ÐÞù?Š¯Ã½ß"?ƒÀq'?ìâùR…ì?®GMµT0?ÃàÌàEŒ?ºÏ^¢w¹ ?¢ÁSÐjD?£Î ´Ö`õ?éç°éÊçù?»ŒSã¾?Æç‰Q"?¨:"ˆ½Y?´øGgÝ.Ñ? Ná+×ÞÊ?秾 [¢?¬‡ì÷NP|?¯ábï¯?"}uá(…w?¥ôywÛÆÊ?ŒàŸl¶Dr?좢9PX³?š×VŠó…ìOTHER4FGL J0844.9-4117¿æP¦•Dd"?ï l¡éÊ4À8ôÃóà7
À:ËeCP·¨@¤d[Ÿ8@±a£Êu?ÁSŒÄôç?Ò`…_@V=>Nð(@Qï x¯?ïÚ¨W¢~E¿Ú"uá-¬á¿éÃ}Ò霿èØRq¼Û¾¿ïÿÿ>¹ú?í쉖WZUNASNone?Л)Ÿ³˜?Âý'6"݆?Æ4絨»B?¼ü¥yîûÃ?â%1‹E÷d?Ƈ®f™Ö?ӏQœÒô?ËÝÍ]íÇ?À]iK&‰?¶¢»ç[.?â üîc܅?ÌtÚìäß?ՓÆd– ?²3n|O?Çíb!:ëÂ?«voeA?Þuˆ‹\ó?²[¨Æ}ëM?Í)àŽ —:?§AJ—欖?Ä|øîFx?ŸxE¯D?㖂]'Ø4?«Ù1Šº?ʕr'9p?¾`¤ژù?ÅY;'?»j†Ç
ý?ä›_bÚ?Ĥ'‹‹?¼á¦ùßç?Á4%	Ùj?Çý0Aç+?ÂÝùÔÜŒ?æ£KòÐJ8?ÈÐÝ{yP¬?̚'eÑH»?­Jíÿ–[s?ÈÿœKei?­i±bw¿5?â™tSËw?²¦<tûT ?®¨Õ­¹:?'¶@ŽM?ÍLÒpG2?¯ñ«ƒJ?æÌ-ý¶œ?±6ÌKÆȔOTHER4FGL J0846.6-4747¿ï?[…6áÀ½g\/«¿À:€vÙ{0ùÀ;¢&äpX@!	¬&9%@|Ą(ï
?Â"O5G_¿µÅ3{W3?ó²"ý[
@T€œGžÐ¿èei|Æ¿éƪß<;¿êúŽÜ§5d¿Ù}®A~6¿äCt~­0¿Ü.Ë$V žUNASNone?âÙØÒJ—?Çj6!¦?|›@ª¢#?©)¹¦Ÿÿ?ÙÙâ–z?Æõ¢¤/IÅ?áÊgq3<?ÈÑy(yµ'?':§˜'?‹ÁӝÂ
a?ÛÙ`y<æ?ÈYè"Ç?åćÔu7»?²}×2‹«`?'Xåpóã?†E|…
zÐ?ÓešÈ‡‡?²/5¬=?ç…pÿéÒ?©Ç"Ýv~?ziHN¾v?fOÎÞsÞ?ЋxÞQô-?©Å"õöâ?Ùòuóø	ç?É6DZ_?Ó,^îýî?³‡ˆ_ørŸ?â€+£5¾m?ɑYLU Ì?ÒÀŠ÷6Ð?Å??êë_¤?¬Úr—œ?ŒØ¹ƒÞ‹*?æ``ϒh½?Åyh̝'?ÞÐ*¦Wÿ,?µy'$Be¼?˜è'Ó1*?Š6Þ©è?ß¡TvØW"?µ‰jÛ½Ü?Ùsì&ëbu?µ,¹Î@¶?l|'é?"ö퍠¯?âÅ&ˆ³uì?µb‡\ŽMIXED4FGL J0847.1-5954?ïý‹x'¿À$••ÝLvÑÀ;cÉ
ûkFÀ< ë'+@!Ù0*Pš?ý«¤C@Çp?Ï-=û¹o?­Çƒêó:?âéóN@Ö?ÿ6±Ú~?»Ò6T/=¿íê͈ê?®%CÜMÉ7¿à¼{Eñ|¿æ¨ÊYUì?ÑÞÖO,þUNASNone?îbSª?ª£È·2i†?D1ý§­Òå?HÅ ¬éÐ?¥ÙP1BY?ª|ïTa+>?èéšQ5¸Û?Â>$,Hø?và%±2Z?'8#˜—Û?Ë¢•'_#ã?ÁÓKâ+®°?îo(6ªáë?"ÒdïÌ^Æ?l¶5R
'(?qxÓ;¼ò?§B=ßKº?"+"7Çñ?î#±ßFÞ?Er÷—i?nz÷qØá¶?WNGɈõ?«Ý2'Ò¿¦?>v)ÊK5?í²6laØ?²é‹XSÍ?L¹Ù*'Õ6?J•¡õD"Þ?²4ØíÊüÇ?²Öe¹Ù…6?âÕ'7/Ú?Ê
¾±kž?y¡nL#?†Ý[·Íˆ?Ùï+ٚ?ÉÝ]51²w?ìµ0ö`R?£LøQñöc?t~k 
U?u=°Øà3?¹'"¨ÎG?¢¼™ön?ê¬÷åx?ªvM˜×·?Dø{¨ø?wD§Ù4?Ƅüœ¦ÇÞ?ªìúûÅnñAGN4FGL J0848.2-4527?Òs&#'f¿ò´óý">6À9OðøûÿÀÀ:ÚßVø4@a±U¢ô·@C›0r?ÁM P+?» 'ÛŠ?Ò2ÚÞ2zÒ@ìIڔ‹"¿îƒ¿<ÁQo?ïéªS%A¿ç¿6ÁÞ[¿ãâ¾°ÕJ¿ê28A:
¿À\Þ'h#ÖUNASNone3FGL J0848.2-4524?Ù^
Â$¹?Ãú§"#Ö?¢",Uö?š>õüI{Å?â'¸.–Q¢?Äg˜†6)?à»^>5#?ÉÅá\bÔ?…1`§¢?‰jé½OT?Ý߸ƒ$ô<?ÉIDŠ§
?Ô¨d5';µ?³I'YÖÎ?²3ô¤,E?Ÿ×ÀL?ãi‡f¢\?³¨Ú9?ãÊÌ©?ªÏ¯+±r?šÃæãéã?yt†H†½?ך'µF@?©ÝOa¶*?Òn,pâl?ÀÔ?DZð?ª\‡ºU?¡VIçoÕ?å#)¯j«?Âч'Ñè?Ò{bßÚW?ŲV´—¡È?Žþè'ÿ±ù?žáRáfqU?æF|,»
Ì?ŗÄNÆY
?Ç}»ÏEð?«Nªïî•?³RXj?¡
ù# }?ç¶xF&™·?°
#çiDã?×õ;ïwû?±yk=$µ?§jÍÓWâ\?ŽÂ~ǪÇ?⎵+Åß?±€Q•ÿ?MIXED4FGL J0848.8-4328?ï]üûœL?Äñ€uÜ%/À8UëºÎ‡À:aŸ®†¨@ƒv‹w—ç@OÅÛAÖ?Áh™ Öd?Ã[#§¤õ@K#@¬	YBg?ïÃ>Ò£¦?â®
ŸOæó¿ê0dKÙó&¿ê†Âùå¿æ¦òèÀHZ¿âÌø6#
UNASNone2FGL J0848.7-4324?Ù°i
?Ðc	r£I?± Òę´?²‡	'Ik»?á³ÙòáE?Òy­%ßÛ?ËMQu=§?Ò]ÿÔOè?¾˜'´4ó?µAª'ŒËZ?åY›P©ø?ÃõòsXû?Ãl֕Öô÷?©y6
ø?·
%‹?«*+Ýg?æ¤\—@à?±zä3uí?ÌÐcm–9?£•ñÆ浪?ÆRú}#,?¢Žõ¤^¿?ã7(…Q°n?©ëµ[œ'?Òa˜Cá´Ä?ÍÂdËÓõØ?Áwæÿ±"%?Á×TKl÷
?âq:™T6?Ó¿oÏV?´"¢È‰Ÿ?³#½žkî?Æ6Æ?ãú?Ã=5ැP?çẜ?ÄÕÌÃÆ‹?¾¢2¿?¤Ç{½Ü1(?Âáë'wÐá?¬Ð戛֜?ç…PØXÑ?±qð»ZÖ?µK¦¸û"?—ވ'?Ï
ÄÌo§$?°ëÕðÈ<?å"ëø62?±ˆj³NrOTHER4FGL J0849.0-2702?ëýt
•e@$óÛYXÀ:¡µÿ*íêÀ<*hþÇÜ@)=Úù@v»cýM?ÍZ÷¾=?Éë9ÊQ}?ú¡:wË@ÙùŒÉQ˜?ïûÜpêN¿ç©µ2&¿é/ýS}U–¿å7ÖeÒ°¿ïÿt¿Å}M?ÙÈÞÁ
XUNASNone?ìuLUC(t?˜ƒUE½á?ƒ¿YNªLå?€¶´PŒÜÞ?¹Ý²*蔇?"}\ø?í€Èµ.?³'Dsh?‹éžVÒ%¥?N<ÿã?°|ˆ?=ÓV?±.ÉÄWý?î
h†¯º¡?—´ã÷á£t?‹Ø"ÿ$?"h€KÞ?¨3n×Ï	h?"<™ö&\?îڑ@&-3?zJ0½o‡+?'Ñfñú?bš×h:ç?›E$½È¤©?u]¦"O¹³?ë«ÆÂǐ?¹Í"n¨®?šš2ÿXP©?–j"£"Œ¿?»D×?¸!0îöu?éË©r!?ÄÿërªAˆ?¡z¶¶}-'?ªnú%ç_?Är®tc?ÂÕCç"?ëfÏFO?¨bù.Rï?¤¦Å2@ó?——âƒo?½|4Xø?¤ao_Né?ì&9¥	±§?˜X—çTòÒ?"¦fˆT‹?ƒ¯gäX?·m	<X¨?"yeiÄFAGN4FGL J0849.2-4410c?íx'àÅ}"¿Ìl‡g½ÔaÀ9ŽËŠ­mŒÀ:ž¾®üØ-@Èíº@òâÆ3U˜?Ú®4Ã?©újꯋÉ?âÁ@Âgîý?ò²jž.~Ã?æ¤ðzPþö?ã²ç®6¿æ]Ç[sÄ¿ìÏÿ‡4<H¿¢Æ¾bHA¿ê\›A9†4UNASNone8?ѐ¾©žt?Ä»=©"?²9{•B_?ÅK½ eí?å8.£U?ÉKƒîÙßQ?˳Ñ[ÛP§?ÇI'»Ìå?–3
›O×?çv¡eù?èasTH?ÆåkE.™'?Ñ!=¢wä"?±QGƟ(?´Þrvb#?¡®²´?äӒì¬;2?²‹jR•_^?ÑÊY½-?°†ƒ•÷O?Ž#…+¹p?€•#¶9·?æ¢E
6…‰?°Ìûivú?Ãô†Ò9Á?¼!±QWq½?¦|eöçÃí?µßb»0ú?é›ëÚA?ÁŠ'kJ÷?º¤fkϜ?¹ï©H8S?››äé«{?¬@ÚÝ#	¯?ëΔ5'?¼Î`JÃr±?ljS÷à"?©Ô!ÌJÊ=?¶ºqÝ©C$?£;4*_ì?çF\Ƴ
â?®íqe£?¼^)œí?¦ú²E.½?Šr­q'¿`?ˆ•æO¸v•?ì
q"Á_?§§uzÕOTHER4FGL J0849.5+2710¿ïé=nÿ½@B`'ݽµÙÀ;:I¥ÒÀ<š…&E'@Ɖˆ*@ þG™Å?Ñd}£Cç`?ÊÙ'#0?öS¡Qô¿@ˆ3û°'¿ïö
~C›?ï•Z0Fð¿èªq"'¿çq'úä¿ëK»%_5¿ïÒŽXUNASNone?ïÍ~^¼?‰d+ga—?jª	
‰R?c!ÖËp"·?‰qH—žl½?‡"°ºƒ°4?ï¿¥ z?z\†"U{?WsSÅá|?`wßwVÉ?zš›ÀÆõ>?tÙöd…?îõ‡;	?S}\ul?{Ð#«@4?|¬vgþ¨z?šYæ,BžÎ?Œ?úGØ|p?ïj-™#?kk '×v?v¦¿·'ë?X"ë''j?ŠTÐ{}Ü?gþÃ<DÈ?î݆¡wç÷?›í O6ç ?y,AC?râj/¬?žŽ>H?™®ùbêY?ï:Ðݗd$?•×霢sÄ?nUeò?{KÞósù?"âÄ‹-?'‹Œn@ƒ?î)3ÛNŶ?˜=»óÕ³?Š™°ŽÕO»?†Ÿˆ2Ӎ?¦ÆV*Íì¯?"eiàE.ñ?î|*ÈMµ?‡ô)'çBÈ?ˆ Öܓ?sÙ¸ÀÖÜ?¢:pfh–?…lmTþAGN4FGL J0850.8-4239?êï:@	? ¯ø×À8È.¤X9}À:OfµN+@ÿ¬)Ü@	}î$nt?Í(+Zå?è}´'l¤@«y"O¶?ù²¬Ñ~¿Øs©ÏqÿÙ'{#â³>¿í*¶W?ö¿ï¬¦Q8ø¿Ý©y¡Á¿ïçÑ­ÝUNASNone3FGL J0851.4-4244?›À~·u_™?¡Àk"ži)?u}¨-ÐW¥?€b}mOùç?î÷¹¨¬?£™Ãøø*È?ÃPT±j?ƃ6¨]­?ÈSGz½á?€
mRz?å$V)5-?Çü—L…?É	ߣzT@?®ˆ>xAÍX?¹Yº
?¥Çԓ¶B×?æ'PÕZî?²l4µk­?›iý,"?·Ã£ÊÊ:?Ô=^ÞeY)?¶)hâ ?å§'"#?µ "¨T%$?'t—yš?—ÏFô"?'ð"_ê,?‹ÑÆ5øÃ?ï Yö2? x­¸x?©0ýŽ`«f?´_Á'ZZê?х³T
{?ÉÉISþQ?åª|Ì·Ý?Éø£6ȶ?ÇçÐáPß¹?®áϏáA?¹¬È=¤ƒá?¦'ˆ–ME?æÐr¿÷7–?²ò0¯«ú?p¼¹Ÿj‰L?`h|À?Ül™¹Ø‡?ÂìE'J3Å?áÜP@	Zr?ÂÔå¦s­ÞOTHER4FGL J0853.1-4407?æ2<	4uí?ֆsa¡…¡À9pNŽÙL7À:ž¢¶xÍq@åÿjþ@Œf«/Ä?Ð%lZþ?áf¦ÈVE‡@ÑÓ¾X•Ã?ÿbÄî‡Å¿èØ?ò‰J¿³ÓÿÆõw¿æ%"CïC¿ì(¬A<
r¿ïÿ|¢gô[?îÜ'éSQUNASNone3FGL J0854.4-4404?ʘÞàÂðL?¾'ÊBXêþ?ÆÆ/'_…Ä?¼¦34Nªø?ã¨<bíò?Å)Ë^h?Ð<ê…ß?NJsgfý¡?»dtý5¨â?¶uý½myÏ?ä'Òë[Y?ÇU^:a¿|?ÒBm@}Ò?²3¡I²b?ÁÎbG·"n?¨ßÖu?âŠF7qÜ;?´'œªò¼³?½Oõz"Å;?¡ØO%•?¿$H
#ÃÃ?Ÿü‡±ñ?èqxO
îà?©'¶À4Ò´?½#¬&Rê?²XsfxÙ?Áæ"}æO?¹
SM@ø?çáâË3<?À½Íê?·¯Ôg¢…ä?¾'-ôãtã?Ä{+vóŸ?Â$ê1Ùä/?çë>§Û{¼?ÅùŠ}-9?ÇW$$ޗâ?¬…¹Hþ¤ö?ÅGª…òj?­x&î†yå?äée&Ým?´dNë2?š¸
Q
?†•¨ÍM?"µ,?«³!ÿÿá?ê…xR!5?­•ÏSˆOTHER4FGL J0853.6-4306?ïä¦i¥yæ?ñ%ð¥)À9
OH<¯´À:'²jJ÷@RÎؕ­Ò@ʁ~áS?Éj )?åÂ:¢"=@I!ßyx?ôIYˆ²l?›ƒi+'«¿ÖO'Ÿ,*«¿èeàš	+"¿îÞ§ msK¿æ©n)©G¿ïù>/GìUNASNone?Ѝ&éÀ·?Å(‹ã+;¡?Уw¿æ?Ék4\å†?ÞϾvc?˛ Ï¥¼Š?¹>5ÂEœ?ÀUAGjo,?Ìó0í;_Û?Ã.~y¾Ä?å›m"?Äë°'ݾ?ˬ8Öhàr?¯UóUçW?Èà»æZj?­Ö7ŽõlL?âÜÂÐÁñI?³9¿~m‰¿?¡Z᫉º?qðT˜àðq?Ӹ۱ʛx?°•­¹§¥?å¥»"?°/:F¡Ù?ÅCÞu°u?½±¬àÉ?Ê÷L÷%2?Ä5ôõq?ãñ5]–n?ȄéÎÖ?›Äµb^*>?¬åét?Ñ|ƒS@?ȑj˜qÉ?æc˜Éˎ?ÈG¼GˆD?ċAÿ¡,Ø?«"mýþUØ?ÉXÄ^¶'?°QŒO.;}?ä†þhj"?´ &´FY†?ib@žùþP?TY%Eiؕ?׫Ǹªš¸?ºÓßòÛ?ä¹ã)õ6?ºÔ¢Õ¾ŸOTHER4FGL J0853.9-5501¿ï¨Å¨ZÀ!º^5?}À:¡îM¯À<
'Á8D@ºSç2Ԕ@þtYœT?Щ•$¿Òé?Ñ*¢ëÒÌ?üíV•8	@ƒt¿±?îûa3v¥¿áÖ!_K?¿äK›^ëÈ¿ç&#€7ÈĿ런9F¿ïöI"]ÍæUNASNone?áW#ߋÊ?¿Ù2©Ôþ?¡Ý‰(J?‹5	
áH?ÛšÖIg?¿C"Õ9­Ì?â¡KiµÑ3?Áô·7_?<+^=?ƒÝvŽ?Ù¹¦|"‡·?Á‰rF»È?êgŸ+*ü?§µÄå¦!?¢äŸÊ‡¹w?".s&(¹?Á¨[Àè_r?¤jø
Ʀ¾?é+½{ª?˜9ИÀH?¡\…£?{#ïÈ?Ç«­²ïñ?–z™iÂ>?ÑóU-•É?¹<:ÒӐÐ?¦ž%šnUÉ?˜Q"9‹Ñ€?åœsŽŠ¿?º7)2ºxž?ҝLñ9,‹?Á}Üjµ¼¡?˜r'k=jä? @D·Á­?åíÄô2¹³?Á•,†ŠŒû?äŒÕ."Û«?°cB_dÙ?³JT‹^$?ŸmÐ+ë°?ÒÀŸ wb?­YÝÎt?áQ.Nz•?§×ÁSu]?­CÃAfZ[?'þ*&"ö9?ÚPå:¬Ï+?§]¯ÖÄ]ÃMIXED4FGL J0854.8-4504¿Â.ù°¹#€¿¡MŸßȖÌÀ8"Š'¾ÙÅÀ;H"ÅõB7@üíåKHÔ@
™#R ?´7¬"ž=?Ý/0ÓÊ@#ƒn—?üL+ín­Þ?êñ"¢A]î¿Û£iüóÜ¿Ê÷Ÿnc‹¿ã´k!a#±¿í]¶>•çÞ¿ïÿ³^¼£àUNASNone3FGL J0854.8-4503?Yÿ:1?T.—c"ªö?îq'çÙ÷
?¢IÉ8ðß?¨yu•a?¡í:MÖ8?ˆ‡ä±.?'½
Ð"?çÒL¬3­µ?º×):>Ó?Ï54ÑT,8?º&AT«u\?Œp*#Xä?‹¯Ÿ) kÎ?ëÆ¥³@?©®WÝ/È?½¬ÎÌùÆ?§˜²‡?Œ"…SG—ó?n £>¤?æŒyû;¤?¤¹µ|zÚ$?Òoށ¢y?¤vÅ+´1ø?b"ŝN
?\ˆ®½%»€?îƒìÐQ?£olˆ4.•?¦§dî£('?¢Ç¸‡b¸Ç?z/Íɇ(?'ÓÚâ'®?çî'öÙªp?ÂP	˜/6N?Ïtuµ[8'?Â7©ð: ?'ùÍxþ X?€`ñ™ú)_?ì?™Ä?ªœƒ)¦Ó¥?»¨?DÓ?©{ÍØ+?nX¤(GÐ?T%çvÃj?æä֊L÷?«Þú€!?Ñù¡¢ã«r?«¾#Î¥ÝPSR4FGL J0855.0+0720?â»tŸ±ƒ@>Åé\îÀ:Ã<«ùjÀ<\R±}»î@
´t:å@¹™Üµx?Èx/çyKp?‹Ì*IP?¾)lµàÍ
@ԆλºV¿Ìєݝ)œ¿è|u éY ¿ç[i³"¿çêï͂Õ2¿íÁ¶ÿ0![¿ïÿï9_JUNASNone?ïgÄ/s?,2ë#»?mç>
¼â
?cÇ3ªÚ85?Ž•$°\«\?Š)¥Žä½?ï´LÏLÀ?~€Ÿùã6î?\æ•oñ.?d¡D'¼ê±?~ØÞ¿ò«z?wq¬|0?ï;]e?‡ƒ 5ž€0?utÍ?äö}?s£`Úź³?–Û\ÈÝóÉ?"KŠžÓ5	?qÃ?fèc:Õ?n©ˆôÞ?RÄÆêÇËç?ƒì¢5Ã?beµOyX?îA%«?¦Åkâ)¿è?ÁáÆî¹?uLoO²/"?§îóò«ò?¥¡¼öƒ"?ï$v=Z:?˜Wqá+Äù?p±ò?Û»?}÷m©ã~?—S­"«Ò?"÷÷÷1 ?î.Þ>(š?•îŸ§Çüü?›ô²Uèi?x´á‡ Ö?¨«ìÉ$H?"%ŸQ'?î҆•ä`ñ?"êj/ŒÔ?ƒözÿ{Nï?q%o†Žº™?›³ïÄ0q?€Çž]ÐJAGN4FGL J0855.0-6026?àa*•ˆp…À#µKjaªÀ:Ï,?#+~À<U™OǾp@Xš]¹Ä‡@ôº¼ÿÐ/?ÏGRúν¾?Ñ*ò‡qxé?ÿV­ÜF½T?ÿt'Ln¿èã'Á¹m?í£†ŒG!¿Ü~óûå¿¿âò(؇¿éÔÈ¿L½¿ïùé€aº/UNASNone?먃Óp?´8\(O'?'ezGÀ-?…ÐUŠ¤rá?Ávêº;?²­äÙ	ÑM?êkÝñã1¾?¿AɅçØc?‡F	=…5x?ŠsO-ÖÝ?ÄÜ'¤šå°?¾Øv+ß?íV/03k?ž¼¾·üª?BíMf^[?…¥ä%ù¶?±f(Ö{\?›S»N[?첗‰ôàè?‡2 , ? —™œAR?x2ƒ5É?²và–Š?ƒq1ľÎl?ä-&°™?šZí%L?£°ãxA?–
ØeÁ­?Õ/—q:Ä?Á¥EЪä?äÅÉÔ±þ?ʋç6Qî?›1.•!Œ?¡{™Ô3?ÔÂÙDŽê?Ê/'C'áµ?éœI҆õþ?­²‰ïFc+? ðˆßO?à?'	u9׬?ÅR¶}¢d'?« cÅô¬À?é
µÂÅ?žÚŠ~g´?­Ž{²—±&?ïÕÇd†|?Äl7p'ä?›)ä–GH¢AGN4FGL J0857.0-4353c?ޚxÈyè
?ð'Ú:s™UÀ95–4ŠKHÀ:}NÏpëû@¿ÃJB~@6&}BJþ?Ò#1=9ÇL?Õ¶¥ä*·d@۔XÖ[?üo|½?æö?ìåÁX¨8¿×"›¾7Ô¿æ"Mºö ¿íG¨€gC†¿æ4óý">6¿ïÿ
Çhß½UNASNone1FGL J0857.7-4345<?à\Œ%›N?ȝ˜Ço?ÂoVYÓÛà?ÁŽ+&³?Ö¡›ºÊÛu?Ǭ0rí?·‹sø¸H?¸åÓ¥Vž?²aëvhå?®i²GÑ«?êËs4;W*?»÷˜gëK¾?͘õ¥7²?¯sõ L'€?Á€'±~ùÁ?ªCùÈç©?ä9ž)ÔÃD?²G¥v'Á¾?²HL%ñ¢?Œ ?ÈdT¶?¼½I•'øu?™Ç#"k{(?êmÃä-?€ä¤¬^?Ôqn°jt?ŔÍ2‰{P?Ã.Ï&Õh
?ÁÃþ¥•"?àû"Þkï?Ê3–ÛNDÜ?¤ùV‡dýt?§¯ýÁá~?·NlH`hŒ?¶K.Ãs?ëƝTgÇ?¸Ãž?ÂhB$£ß?¥8?¥ZK?Ãäd:‰‹&?°D\W°X?ælÖh4¥W?²ïêۖï9?'tdí½N?uu{xåx¤?¿ÏˆBHØ?¦0.a‹aþ?ëzkÏíú«?¥û雿­MIXED4FGL J0857.7-4507¿ßpà¢â‡?Ôð°lCõùÀ9_É'%Þ·À:¯"¡@ÿi«kG@%³Æk‰¼?ÍÙB¼h%®?­N—½¡a?ýäJ|ûÔ!?þ`Z³«¿äý ¿¨¡õ?ï
}—"ã¿ëfx¿âyì?®ÁŸ¿î–#ùŒ|¿ïÃOÀ²0UNASNone?Épù"xië?¹Õ­9<?T?¨,ŒÃÛ?¥¡õ!™qš?è#>ل–'?¼³òÇnzB?Àîs]Jx?¼Ì¦CB—L?²í83??ªŒz(8y?é"@ë=âJ?¾¿P.ãå?Ñj¹‡J¸?±#ëu7L?¶ãK]Þ?¢Q91é Ý?äcá?0ә?²NaýjV?Ì·afÞl™?¤Ñ
×Ç?·r®€'úè?"<sè…?åãÑÖCe}?¦ðu'íÁ?¼\­H*Ä­?°&H™­ØÄ?¯Ï~Wô³œ?¬	l"X"?êwrq{\1?¶Xÿ}D.?²Áån'|¦?±Ygø¨@þ?ºû¿­Ä7Â?»Jµ}GJå?êHK\0Ó?À·¬I
?Æ¢aÛ"Œ-?¨½'—'à€?·s¾¨A´?¢ÃÍØb§?çhﴝñ?¯ôÀ­jíñ?¶®ªº¶?šo=ŠÑ?¼ðpDO?¡ãҋžFa?錠l?§êº[OTHER4FGL J0859.2-4729¿ã×:@š¿ðn*¦€2À8ŒÓa;";À:'
—~6@&®¥Ô@Âä›ök,?¶À:Çý?ÅÍÛÕÿ%@
èþüÊÁZ@ße»Æ•?ìäÀ™+¶¿ÚŠžc˜V¿æŠâ¡ö4z¿çì2"'û@¿é"¤!²Ø/¿ëbZ¾ž
UNASNone3FGL J0859.3-4732?ϐ¡å¢?À"ñ·Æ]û?ËjEÁÞº¿?Áºë›;}?áAFO€×è?Ĕ|ïiÚº?Èæ»z-Ý?¼;(ŽÙ;?¶ú¡œGsÝ?¨z%‰G)?çr˜†
?¼~+®Hl?Ì}9Ák?®°:n0¢D?Åg´†Ò9?«2À^?ã†Äm‹Q`?²zãmž?À¶&hۜÚ?—Å´äû?¾;ªÌ­ÿ=?',,ml ,?è©è'?Ÿ³'O°Tb?½â®/†^?·"¾Èõt-?ÐPJg¤¡?À‰'?>?'?ä6¥<ä?Ð:%ÑÜè?­gú*'?¥ÑYo,?¸¼}%°î¿?²ë-ìê}?ëþˀ$0?´ôîž^_?…)C´úb?§]8)ä?Æ÷\œ§Ú¿?®¥b>í?å Þ‡èʸ?² hçBÅ?£È*àCñ?…<]kz~J?Ą×ìï
?¡¦ŽjS•Z?é¢{÷¶õ?£¿DÏÂêYOTHER4FGL J0859.3-4342?×-rKn`?÷]qËväÀ8¤ç2© xÀ:Š·y¥@‡BÈÒlI@쭀k`?»@|`½sØ?عïºãkJ@9#'Õ?ö‡ÌbCÁ÷?å°8!Y–õ¿ß|÷7¢L¿ç\ž ¼ã÷¿êWÕÿïýÄòã¸?Уi&4G/UNASNone?®#P¸»Y?ªÚ€mm®?å¯+ÎSÏO?ÊgL×ì]?ÐÝ>LÊfŸ?È0*ë?§yb	Vã?¯txŸm?ÛüX? 8?Æ£"3m?àŠBŠO_ö?ƟÅâÑú?ÁöûnÀ&?­§~Äu?ái)‰]®©?¹¦±ÉÕæ@?Ô2/6=Bš?´¶J-ºg3?''«ÀÐ¥?r]ÿ<q,‹?ÚôƒB¼ò?§²ÖGô0?áü†E\'?§¡ÌŸÔ'Õ?¡`8óé%±?›w¿'=`?æþüwŠP&?ÇíöyT¼?Ï«ÿåJi}?Åç–ÿ­Â?‹¼—ÿÃ<?šè$?ß¾ö‡¨¢Ã?̙ìý¼%W?ßc$¿Ÿ_#?ÌH
AÔX)?³µ"¼ù?£ÉÔ½	Ÿâ?ä²Wºfý?¼
ÞbBâ ?Ñ®
¦Ô)?·S¨)Õ3?g'hÒ?Q+"ïp¸?à‰nåL1?³CL/–a$?ߘž#Žqë?³9Ë­náÖMIXED4FGL J0859.8+0053¿Ï—¥»2gÿ@<®Ü]cˆfÀ;9!‰½"À<¸d(ž"»@"¢ªÜâïy?Ô*"}ÙI³?íEÝYâÊ?ïÿÕ7ÕYc@žÁÁÖυ@B)"â?ì»m߁…Q¿Ó–Ñþèk¿ïÿ4Þ®÷z?ïñ
žÏ
š?Ù·`9{¢¿ãÊ?wåUNASNone?ï"\?¦§ÜUëiÒ?Ž¢C8]5?¤"ì¢ûÏ?Ž[ö³ü? Þ÷掼?ïl'εkm?œÚAQ}I?näYRJ?¼S®öÎ?"6ûXx?—uÎÄë?îÿjœw?ž®"‰†½N?'
ƒ;´6(?'ÄÙWW|T?¦ºÇ·p6w?˜?0‡"O?î"0
[T²?™@®¼ƒð?:ùcûVüa?NF¬UäÔE?¦—d{ûZ?™Mþ8ö-Ô?îƒà¤ø?¥œÈΗù?ž
uŒÞ›?£F#3?'nÞía?Žël㹏?îºÒæäp?¯TEIݯù?S)(ˆd?™/;rk9? hlnöÕJ?©êÉ­ œ?ípÂ:Öa?¡]*ç*L?Žé÷{?"äÎpÿ?°œËG#›Š?ž·:§6^c?ì°çqœX?³¸{O4ND?F?tlw\§?eËOƒOÈ?ºLE†z‹•?³·:z|'AGN4FGL J0859.8-4530c¿ë®ÇÃoù/?Öù¾'BÀ9.Ž'uÏÀ:§†S€@O›æ¥ç@¸1ôo?ÔùAÀÖÌ?î¨Ä_@x@£ßm¹@ÿ?þN>&I¿Ê"ù#—ß°¿ÅuB⨬1¿ígß7]¿çڙz"¿×¼Zcα~¿ïûï¯OäUNASNone1?¶ø‡å·áK?´ñ"n-ñZ?¹­9tú¹?¿2Á‰˜£?éëGÔªç ?ÃÑ2Jˆ—ò?ÐÑ`"Y,±?Ê1‹w[Åè?¹ÜêšEĎ?¶À—°zï?ä[²bŠ±?ÈyfØ@N?Ô¨·¡8ì¨?²Ö
‹t?ÀÉ&ôzTŸ?©Ï8Ć?áyZrDô"?³ê;÷S¾V?ÁVÁû?§ŒŒp¤?Äv€i5½k?±–ZZ¸‰ÿ?æž|ä?¶À{GÙd?¹
¶L"h?µ>‹½?Á'nø¹Ã8?ÀP3ÀîÈ?è~
pF5?Ä÷–Ã(?¸b`E°¦`?À\ÜqQô?Ç¿&PÌ¡.?ÆùE_ÊYÅ?çêci9ˆ?ÉE;=ïî?Ï~Û¡ÀžZ?°ÞB6£ƒ'?¸W0§¤?­ÓFdm†Ï?ãr3VC®?´"R0£m? ü^=€œ¦?'+4¼>B?Îì>µ¥òK?Á›8þ׿x?ç5*n¾y£?ÁÙtzü¡OTHER4FGL J0900.2-4608¿ïÿºÄÑDš¿†* Û[ À:Ž‹µ«HÀ<hõŒßw@a~#òM@'ª\_|g?Ò|Jž‰Ãc?æüÑA¦"}@	âšÛ¸ù?þUºêw,²¿èÌâÑñϼ¿å¿SÒå낿ӷè99Ýq¿åÇ¢'¿î2ÜÌQ¿ïÿ'Þt†UNASNone
?É#ÛÁ 5?¾ýg87C?Ë^E'}½è?¾´UBã¼?âàå¤pHy?ŗ¿MsÚ?¸jSýJq}?·I<s0 È?·ªü=¤?±µÀD<ì?êÀ äHŒ?»È´Íìª?ã?þXò?²-ôÄöZ3?ÃFt§Ð?¨BL0Ô5?ÐGÝ"Çâ?­±¡Ý'¿P?ØcFë2k?«Pº#D+=?ÐåChVøØ?ª<¹5y?Ö·uÓýÔ¾?­‡îC¼ƒ¯?Á­è]Ctk?µ=uãN?ÑvLcä_?ÁÛ÷•«Öç?âمB}0¶?Ä¢C_-ë~?¦ñ&ŒEmÿ?¨¤ÊÇ2?¸_ˆ1l}?¶æcj&?ë"ü×®?¹O¬½°´?ے?k-~?´l=ö…­Ô?Ìõ–ýÛ§?³Ê¦,g §?Õòõ…Ó"?²Z—Âë&É?À?·ƒ»®?£k¤woØh?××£dˆ¾?·Vc·Íq?à@†O\V?·óTpc£MIXED4FGL J0902.5-4727¿ÔJNd´W¿âŒ0êÄ/À9—áZùJÚÀ:Ëu$oK@ =¢wä"@U
`¬B?ÆíÂ;?…Õ£òQ5?ÄøŸ£ô¼U@ÅKSuÙ¿íék¾êáá?ïî5gÀÙz¿èQˆ˜`´¿é5#˜‹| ¿á§a8)<9¿ÛoÑ~ã4îUNASNone1FGL J0902.5-4731c?×}C™?Â:-ìUô?‰Ü¼ZÄÁ?'€qÑêÉ?ãØ΋œ^y?Â^ËH‹	?Ðõü^¾Yö?Ë
γVÀ?ˆ?æ
ÕD"?à*‡·?ç$8i}ó?ʝì~\Á?Ô½ˆ0æ|Ì?³šu¯vÔ?±FÇ'f¥? "µ‹	¥?ãxk®q9v?´>PpŽf?â|TS-=j?«Ë›I(/?"ž›i°ü??j%	98ªœ?Úbb~WýK?«òœj.?Í%Óæ¾ÝÃ?¾p̓½—?ŒìÑ*þ§?…ŠÊÙ3‹¾?èF?RâaE?¿ȨOêÏ?ȖñÃ,Ò?ÃüpBL?‡9nRòTì?—ú'ãUƒ?é}]Õ·ñ¸?ÂþKÞEV?Ç\"[t›?«!÷ße¤Ì?²tmÙw?¢¦<‹¾¾?çÚxÓ6¯{?°(­?¶Ñ?Ô7òjk-Ë?°Êi"áßâ?U'—?ð€Cy×Ó?åa^Uå~Ž?°ØøÉËVMIXED4FGL J0903.5+4057?ÑÂz_¼@DÚË}At?À;­RÜEæ"À=û¼¤`@ {åóìÌ?û¾Îø 7®?޼ɴêWø?ÆÂx¡[?íìw¢xæF@â!Üɚ¿ïÿ€H»Ê?ïõæ °Ï–¿ã¡Çe"¿¿Ø»;ÀJˆd¿Ñ5¡l犿ðUNASNone?ïÄޜ¶#?xãtݹ5l?T`T¤S#?P°J)³y?xx3ß?vh¾øYK?ïÝFÝnÊ?l¯ü[æE?@"J…¶,x?H5ô $Éö?n±j¶w3à?h•…©ø?î÷Ô²kÄì?'óYŒ4íx?hÀ×Gn©?p@\AÄxo?íNÉýê›?'€æ+%¤?ïÁ|ó#VO?]S8¥%?ME}©º™ ?9»nÏ@B"?{˜Öª43?\KÇå?½Fûp?‹r<覍—?d2¾~`o5?jQ 	ãí?Š‰áANK?‡9³ô¬æ?ï'_ÝF}Ï?‡§X@€E,?RÔ¯óäÅè?^è/Ÿlü´?‰Mr¦E"?…¦2l)m
?îHz˜!Ÿ?›¥ÿ*-€5?r:šxƒù?t;á‹Ø\>?«Ô&CœÉ
?š©¹°
/?ïhاTð?z§aÊr™î?Rv
­äw?T,eô<Z?'½ŠE°ç©?yãÐ[ïAGN4FGL J0904.6+5200¿î²°%]@D§<`ŸÀ;X*CbÀ<Â?Úác@?o¾Â@ÚCä'?ÊÇãÍ¿¡6rWá=r?Õ[¥BDH@
ûx¹ u?ïõõòðM¿éÑ(| ¿àœúAzÓ¿î›;ùç¿ïÐlÊ-¶?ïÎèӓUNASNone?ïóx~u?^ Šƒ?.3^Ûà?3¯Šæ.7î?V3Žb,ê ?Zîüš–Sõ?ï™db€'Ù?Š™@ûo?b[Á¼Lã?n²Nt×¼?…öú(§?…Â5ºº
?îÖj;k?"{«‹ÎC´?v#;³#GG?aé¡C?Ÿ´CÎgÕÈ?'¿'‡SQÿ?ï忀š*t?O}Á=0vu?@äl0#s³?-?¶÷i?fd?FE?M‡jj4ö?ïÐ%×ÕêX?ƒ†¦á?EúGõ0³?Né*./pä?u-Ë$4|?'
­¨õK)?ïRS¬G?¥Žêè6wÆ?j¡y6Ϭ?}̐¹	š2?œÕ%[»/?£ó7ĸ7\?íõ&ÁŒþ?ž DtøE?xÌ8.òë?~ÈØpùÎ?­"êXªº?€ÆÓ¨M?§Y÷?vJ;Ù/À?[^2Én?RQFâ?‡rŒgìs<?uSl¹AGN4FGL J0906.1-1011?ëæåÛD@7ä=F²køÀ;ÙÙ$ÉäÀ<­¶‡*@üÎí¹Vx@Vçæ-Æã?ÇyåHn¯?¥³Ûd?D¹?àE†6`å?ñ¸'Æ@Á'?ïÿWߣ¿êw?&±p¿á"g¾U:Å¿âvYޘ§+¿æx²™Dà?™ü%]1šUNASNone?ï£èyY?¡bÙK?P~mÊU?Køéê™Ñm?›ã·†$Øä? àh
Ÿ??î²'»B¦?£×¤Ú¨L?†¸À4êÁ ?Xh³Y?ž`m¯Ú}? 92yðt?î•ÁÅK"?—&aú­?s0CyÝRµ?u4 B¾Š ?¤I»qýÿ?–ÂwKu{+?í+¤Úÿ?¤å»?–7T'8j?v?¨zEµÿ?±6ñ­?Œžð±Þ~?ó‡/? sûN<ì?]WãÜ}ØÀ?UÀ
rýÔÿ?¤ÛªæME? EÝ¼?ì@öo)ûÉ?ºÐUCB?Ÿ©=‡'3ˆ?¦›K嘻?¶
ý"¥ÓV?´Ý,=Ì*?íÎì»Ìí?œ_EÝEE#?~SxÄS(á?zæ…ùW'?¯UbÎə?›Dq#?èMñz&?¥áÐÊEN?ªAl¢cÄU?"æå=65T?É>mêýÔ?¥ª"ÀPbzAGN4FGL J0906.2-5337¿ï÷o{kŽÍÀ"?Åè­À;ƒÉØ)øÀ<žæs.Ì@#XîßFL?ärÈ^þèÿ?ôP|V?ïõJšX{@["UU@ӌ1Q0Ê¿ïþÜêQB?ï˜Ê õîÚ¿ð?ïÿÿ&¦³?êbÙHÜä¿àC ´UNASNone?é<,æŠZ"?ÆÕì×ÀW?ˆ#sï	9?¦"hŒ™F‡?ɍn)±Þ?ÅÿϨ
>œ?æóLn‡a?ЬÏ̆€ã?yRÞ\+L?"îæwúª¯?Ñ´§_ˆ"Q?ÐN:P*?êõ 'þ Ø?¨×€)†?œ±,
ß|ß?–L~QÍO?À"YÞŸÆ?¦\¤:âv?ïB'¢7*—?À …Ë?š"ÆÛù?7+Z.D@?—˜hH?&}àY?ænÄü?Ë€F®²}?'©P°lzð?œRNKǚ?Ò°Jɇ?ʲ2d"¶±?àìR:µ;?ÒP¯!#?…"FÅìpÈ?¤î8»ßôÛ?ÝzÁ½$8D?Ñìé`3úâ?é¸uk«¹?­ËôË—¦?ž¹
'j4ú?—DÊB*ˆ?ÇÕüãã6=?«Ù'ÓG	?íù5N҇2?°ɸ`Ó+?3Ž£³Þ8?aÊ^A®"?°"ÆæFê?°WÕI¶AGN4FGL J0906.8-2122¿èŸCYÆðÀ@1.¿üÚ±'À:'ŏÁªÀ<NÐ& û@F»Å™5@ÎC$Aþ¨?Ä°uh·Ïe?ﶰËåF@@Vý<×!?ýÐ$ˆu…¿Øå#»qп±áêìžF¿è×Obîœj™Ñ;¿é>"Õ½6W¿ïk|»<'UNASNone?ÅB¯˜ð'?ÂWÜnð?ç4ŽC«?È#åÖf²?»ÙÌ\£?¹ý4;Ïl˜?¡YA
?¬ÎoS
Þ?ìíH½Þó@?µVÿÈÐþ[?¯Ò3'Ïþ?¬"ý5e
?Ý>‹²¦0?¸]¯ýÙì?ÙiºâG?¶Ôw*_Î<?ÃIÒ$ï?©E9¢¼l¨?§—C¢÷«?tê_E:?ì…!<ª? Ð¨†v›?°TJܧs?–ªäÚ/—å?À+¹c°ËÝ?º™%H—|?ç`Švæç*?Ç#",J?ÂRÀ³—z?¿>&'w!±?'…	y,e?¤¼?S?í¼>ð*ÊÚ?³ZÁqUÖí?ªùŒA™à?¬q1o´yâ?ؗU†1?¸(×x•?ÜRyc]?¸@½‰}?ÆÈ°(ã¾?¬+ϳÿBã?|Ԑ–¶A?sp-w 	Ã?î){¿Ç‰J?¡Ï¸¢cæ±?©Í²ó£?Ÿó-¹ÀŽMMIXED4FGL J0910.1-1816¿ÎöÿlB"›@3¿.Y¯ž¿À;)t"&"À<™™'óe@ U'}‹Q?ú€3çŽ3?Õ?¹=ùµ¹?áÒáïsÁ@¦"¦óõ@N·[÷M?îÖì
µÃ¿ïûÉeeà?ï³t'Ü¿¿Ý~ŽÑ¿{¿ïømÏç3€?ïk²ÖuUNASNone?ï}"´¤¦­?"‰5J¹?oí´Ï"$ü?fh¢‰·ä/?ˆ»å³skz?Ô]½-ô?î^QVßµ³?¨Ã["Õ0ã?'Ç°b›Ç?—épŒÿ5? ·_ÚÚL?¡A5ùÏ?í:o±­{h?¡µ×žÕ:?'x›<ôâq?ŽãOR¿?±Ž[¢èø§?Ÿ¸^¹pdò?ìç>î9?˜peÍøŽ?‹]Açy^?{ô¦5«?µ[oO̤'?–åˆPt?–šÆ?œ±3Ìݪ?‰®âof:?…÷WÝ.V? ÙŽ®"?˜\扚?ì'…@#å?¹ö"}û¥Ë?¥U$I¶W?­Gbkå>N?´A«m—ã*?±ÒŠå)m•?ëŽ8>Æö?§À"¥Öù'?šÀã>ç?'ÆÅVß]?¼ßn½øÉ?¥*c6ù??è9nv'h?±eۀ˕¶?•á+Á‰S¥?­€võå&?Ì]d̪µm?±ûžõ¸¤AGN4FGL J0910.9+6055¿ì}èU¿O6@D:Ü
²À;€Åt÷TÀ<îÈ8–@³Bâþ'?üiÇ)Ý;?Ô¥:´e?Õ¥óD/Ú¹?ÿîãª2n@·7œ¤eû?ïÿÿ^ðP`¿íõGàiaÃ?×de$œía¿ãí:`Nq¿àq9~%õ³¿ðUNASNone?ïFVH›?Žt¯câ%ð?WzRá·0'?T¥Li0ä?‰? !>±D?,;¢CÝ?ïn{ì	¨ö?‰ÈSÁH4L?mª%¯Ño?qoG'\/?Œö{¢Ô
?"<Âgʇ?î>¯Ë¼5?™s
\Ñòc?|J²ÛÓދ?qBz½¸?¨‹¬øÅCÚ?˜TzA¸?îý¬Œ/T?xÖª™—i?oÎ:Cö_z?Wæ&qx"/?œP§5¯&ƒ?ví³YV±?ïo²•i?™@¾øSh?et¹÷QB?azz²Ç?›ãrlZÐ?˜KÈÞ¶?î /ó;p?¡r vüd?{–=åÚã?…²~S(WH?¢Š9_?œÕÕ@+Ä?íSiú? Ò÷×dÙ?€Âô-¨Ÿ?€7E`
B€?³O½$r¬ï? 2§¢¶?íCÁ™ÏÇ?—U-˜d?xùŸƒA¬?nšêÙ¨r?´Ra7,°ñ?–œ‰\6lAGN4FGL J0911.6-4738c?èH'`²j?ۀWÿ|ÙÀ9
!¯éÀ:ÅËÉdc@O9k²r@V½+o"?Ñ,B]ó{7?θ3b­õ?ú|°Švæç?úr¿¨X¤?ïïwâd¹"¿ÐØ
]5»#¿ìk–@ô'ã¿ç©&¿ÝP(¿é«Þ…_?Šú)"ç8'UNASNone%?ྶ±Näa?ƙ‰¸iØ%?¯#ýŒèn.?ª;̔*µ?ڞëü#8?Æ6óäØv?زdS2 ?Ê#²Ê[ó?¬
è™-¤X?¥yúÈסq?áåïLöË?É[ºó¨Ñ?Ôä͸7Çö?±…ùêoÙ?¼n¡÷ñ?¥«ðÍÌñ?áÿÅåã?²Ø²^´?ד[…"û?©e%1?¿Çó½/(•?˜NrÁÍò?à=SÅÏØp?ª˜hFYcp?×Ë!Ô{Ë?ÄZô "?»Ðò n_"?´~§L?à Q2ö*?ł4B|Ò9?Ía?Â	a'¸?¹Ïô'7Z?»æB
f‹?ç¥P÷5Îe?Æè2ñfV™?Îe¶àsÀ?­Q1(Ÿ?®Îß÷w?¬Ž¯þÝV?ãÂf"+?²ó'c¬?Á‰¾-*c4?¡ön9w"ª?ƆÀïz?«{]á‹	"?åûà9wV4?¯±//¿÷MIXED4FGL J0914.5+6845?îÆÉ@	ì@BìÖÜGªÀ;ehžOÀ<ñ¼‡Û+4@! XÐ{®?÷#ք³ž?ÙúõÕÒó?Îf!‡+?ó–*C hÁ@Ãà`¨a^¿ã³!ž¶9¿êZ·D¥K¿èts¿ë<ú¿ÑUíýôâë?'Vä#'»»¿ë5tV2UNASNone?ïØ{…÷8?fnßð4ÂÀ?G…‰`Äbª?;rb+S‡w?pыì'r?d|w‹Ûø…?ïÅ•þ?îÑ£ÕÁ?M§
ÄÂô?[)¢Q(Z ?yÎ?(·ì¯?zÜ÷E¨÷ø?îúæɑô?[;ƒòdø?kϯ¡áñ0?nö:Ø?Eí.ök?‹ßd­hS]?ï·>|I°?d:!Šyv%?9¤Óäðr?-Ið@Ì?c:Hæw¾?cïÖöÊ×?ïžÑÑ2Pú?ƒg¡#¤"?VÊK§Ä?M
[Ïl•®?…‰²c'?' ™²Öòå?ï]©ÅÐs?"~Dò%á?\åÁèH÷?pyqßU
?'|k7:ç£?'ªUcÃ?î]°E"?—ÇǗhBÞ?sA/P̵t?uvjík>?¬FD70{š?–ìȾëЮ?ï%±ÖYñì?ƒÅ¸}Å;?FVWÔÝM?H›VâJë?š—t¯{ï?ƒ™/­hAGN4FGL J0916.9+7756¿ìxö‹Y‡R@@åñà'Œ7À;ž«ôÌÀ=
àj8'þ@kg|×@v8äM?ËÝ
▸"¿µô<'x"ç?ækøÉ6@ͯö¨=¿ïyªæÈ÷U?ïý÷²S¤Ã¿å¼\aÕ²ú¿èL¶Ç§ÉÞ¿Ý}°6Ä¿Ð4'cšY2UNASNone?ë%ð%Ü!m?Ô¬1°Àì^?aûF"rG?ƒ
TÒs4•?Ã#Ï{[s¢?Ô »?ïÄM5ח?€'yp¡.?Q+ÌóGdµ?eQz.	÷§?yŽqòßy®?xD)à¯?îœè»ë©?•ÿ磵?¸kyõ1>?"ùð}sK¼?¡ÃYbp-R?"ƒíç£?ïÐ+'²"?ZFk.ðÙ?Z
vÅãZ?FQ‹èFÂ?qfÙCØô?WŽ"|ˆý?í¤§¿¢?ÄÏS9ãÑv?r?<ëÀ›M?‰År
Ú W?¶³g]ï:?Āíl:Ìì?ï`Ç1œ?'4òÈVgã?ai}bê?osÔŒ$y?'¹ê4 Iö?Žhå õ{¿?íÔQˆUEú?&æ7›¼x?‰('ïæ¶?ˆuÛñ¥A?¬t]p¯¦²?™§
µ)†Ñ?ïd&jDcÕ?| 9æ;—à?qbÑÞÉß?eÅX»‹7}?ŽDüòç?y狃n"AGN4FGL J0917.9-4755?ïB´‹ô{¤?ÀIܘÀ8ôIÐ-ª]À:À4¦Ð¹Á@P'˜÷@#9¾?ǾØWðVë?ÓéÄKd­@èñƒez®@e«…ÕA¿Ô0÷б^¿á§—Sn<¿êœ…ÂL@J¿èà"¿íÁ9¿ì?û}º@¿ïÿ""ÆUNASNone?ÒæðĬ?Ã$†Åßü2?Ëýa9¶ì?À–kÓÉ?ß^¹Qxv?Æk`g/d?Ƥѝ¹[M?Ãt¬ß5sï?ÂO!y*?º½ï™?åÃ:Д
?Æ=
ç(‡w?Ӊs•½°¿?±vôƬpc?ÃeTœm?©ž½UA˜)?ábàƒ|¼?²îÄØÝ][?ÏK…v€?¡À¼¾kb?Ê8i2ɀè?£´LÀ{o]?áŸOoÿÂ?§¿¯î&Ü?Ê/î`¬yV?½Qlçw?Б°Š)—²?ÂÚy';ÈÈ?á+,"ÀÒ?Æ$3†?IÂ?±Å0â{)?²±@ÄÛ?Éã&^Ã?Äã'YW¬‡?çdÝÓìaú?Æí ÎÆeï?ÆòTŽÖ$Ã?«dÖüøû?Å°—(s?®ÌÇ¹ƒ?ä×EGš?´ÀO}!.?°þÕáÖ?'OÞßQÈ?ӋjՔz)?±ÐÙ£Yh?äoØކ'?±«Rµ¡»fOTHER4FGL J0919.3+6607¿ïþ2íN^@C¨ów[0À;$¬þÑ+×À<Ä +"I@ 5cqw'@V#£s7?ËöJŸ‹v?q$Ã-è?Ÿñvû4@ãæé¸l¿èòžm"׿à]àñFÿ™¿è@å¾5ZU¿ÎºE¡ô¿â}a?5¿ÛÂ;yRÒ5UNASNone3FGL J0919.4+6604?îzª$§2?ŒE×'q?TÁ»ß-9W?z-|[ù?§¯Pküs?Å7èØ#˕?ïÒÚ»Lò¢?nƒaYnSÃ?BbFS›èd?Hx,… šð?tFYø?kX˜†ÂÑõ?î×5r
õ?" eY®Ä?`Ðò
úP?iÆKVÕ·?¡¨Ò}®?"a}5šG"?ﶃ?4{?`ð#ÐÔî(?Q»;õ‰?4ãm?š'2?€'ȶ¬?`¿©âàµ?ï'ɯ?µ
Âc­È?S'%%ª¼³?'
0ãuL]?›%yÃ,¾d?´
–÷Ý?ï€Âì½?‡ÐFq+û×?RjVè†p?[…6_áZ¯?¬De6oç?†Š €ÈÐ?î™ú@|?9<­G…×?fñÛ&8K?k5
ù®,N?¬·B§éjG?œÃ-–Û?ïÛCÒ¹?Œù¹Ë?i)ø3ôGg?V`ÁK9?›?XŠpÛ?ˆ$z~cmAGN4FGL J0919.5-6203¿Ý`—ûõGÀ!tBÇû¬´À;,¥R4€:À<øðž³µ@u†6:y¤?üÅ㤧?Ò
 $Ð?è1³¡'œ'@ü™˜f"@8ªÄbC¿ïþ$}㰔?ïÿ5Ÿôým?ßnD¡o¦×¿Þ!ÂÝà›a¿ïÿ胸›¿ë©ââÔ?UNASNone?Ò¯6ÿ›%?Âï§ÔVE?àÊ~ÿÿ?Ʊ†¨Ú?Çw"ÉU?½ÚÙ]‡?ÌÆÿ¬%Àâ?Ç
@ÅÂíP?Ô­)˜Cœý?DzÌÛ-t?ÜïV–¡Ô?ÇÈé2.?ځ-¡ÌË?´¢sà[ü©?Ú_]¼¯Ú?¶›ý€—0?Æ>†cµ?¬ADLméS?æ¶"òÿ£?ªa^ÇdÑ?͘¡
ý?ªhòP͟q?µv´žJò?"1_­ì`1?Êd"ü)d[?½Ž&ÒZ]ø?အ2•(œ?ÆєlPO?Ϙç9ù6?Ã~øÁÐÍì?ÂïÜ`,T?Ãî^ž
?ך
'¥?εÀóOÃ?ßxwÃäyo?ÎW%‰Z?ÐÇGÊvS?´haúW/Î?á{cÊ;P?»W*Á,µ?ȃâÅ~ò?±8xBY•?àR\¼¢è?·r¦Ö02?ÕÚM¶8®?º›­´Èbõ?Ä|ØrO?§¿t øMIXED4FGL J0924.1-5202c¿èŒš5Üìç¿ój
ÃödÀ9+ú—á2µÀ;#"i†¬@9ñ–°±
@C«»Û
?Ë®™Æe)¥?¿g­Ÿq0*?ôTÿ†]|³?ô(|P]?ïúI<‰ô
¿ã1T?v¿ìˆè6ú¿ãÓW€o|¿ïØjÅp·ù?é°â`‡ÕUNASNone3FGL J0923.8-5154$?èÙN¢?Èl¦(j¤±?ž¿yµËê?± lìÜDŒ?Ë÷'fÅ0÷?Æuˆv _?áÃKŠ©"	?Ìc'Ô[ë?¤
ҋ»{?¥µŸ+üH–?Ùø˜ãÕí?Êÿ˜ÃÁò?á~A	ƹ?³DƒßëYø?´1Êr'é?¢"£çýà?ØÖÃKØ?² .†–«ª?áqIéO†È?³ŠÓ+?·@³ânù?˜Ú¸ð7e;?×M?jñ\ñ?³šXÊ053?äYh¤Y;0?ÊL#(<ùÊ?®Ò=ù*Ý?´²@L;æã?Óræ÷ñ=Å?Çôo
YD?Íp'î)"Í?ÈÓPƒ"äB?²Ñ–šÙ?»ŽR:?æI¸1y
¢?Ë0 HÆa?ÚPK™[†?±Ë›üù¤í?¾vð2"·?§,ŠÈQ…1?Þ)œøYÿŒ?²Yìr"ø?ÐOŠ{]]B?³›'(à>²?Ä«%SÃ:?°Ô‰ÊN?â­q|¼`?»…ÊÅ5©°MIXED4FGL J0926.1-5336?Û"™Wª`çÀ蚈¬âÀ:"hZ\lèÀ<P+žê;s@sCC¡•?ûŽ‡Lû‹?ҏ—U»?ç€ISQ·@
ͦ‹ðd@]aXµxÈ¿ïø|}ÿà ?ÁòSD¿À©çÚð&¿×°³Ü»Ø3¿ëþYl'à¿è¡a«ÃUNASNone?Þ?Zې+~?ÄÊ<NºÎ?ÃR`·2"?µû
»Aup?ØtÈ¡;q?Å¸lí–?ÓÜyVòÅ?ÅTëPڂ?ºY÷Õö'?¶Z¬)+Vø?ã'ïÄYÇÙ?Ä
Æ^–Ü?äiëb}èR?³¿Jïl¨Ø?ÁÙ¯ò"?§ý1YïS˜?Ì~¢ƒ‰H$?¯C¯²S³?çGR-? vѝµì?À½=–A(?™Ã%…ÕÕP?ÃAÎaLv%?˜,‡"å¥?ӊ¡±7'`?Áå"[Ž"y?̖n°¦•D?½ñ=xÊ?Þ*&õbB??śS׏ì?ÀÆÆ[Ê?»]Ïå—/B?¾°‡ê#?¾\¾\qšø?è8gûfé?ÂsS\¦ýŽ?Ürz5{7?¶Â¯a?Ë­óaÈ-?²25š1=;?Õ·]Œ ²?µÇì˜c?áõ^'ZÜ?¬Íz-ÙÝ ?Ș«s«?­ üt¼2?Ñzî`ñ2?ªîâAñ?‡MIXED4FGL J0928.3-2713?ç~gá³H@0úZxòZ%À;‹n]«­À<nÒæÂAY@ól¶6³E@w³•Ä"?dž<š«? ûéoð©?×=ÐE'Q~@càη]¥¿æLä_:£¿ã;¦i‹´Õ¿çš
¢ñ10¿ï÷Í⠜?ïŽÿªo«¿ïú#|ÜÊqUNASNone?ïÓ«˜O?p‰Y2Þá?<–—~¦?=û£â,…?taØÍù«?oÈ	yêgh?ï#aý?²("ÊÓÃú?d¨Ì/Þû?yîs"(-?˜þÂÃRˆ`?±‰Rˆ9Õ!?îξ¨X	"?•v"|–v?rn¿™âÚ?{¥½ÿ~u? ÆT'?"#ԝ0?ïîko²ù?PŠ»¦k >øÔt–@c	>ú,–<
á7?abç ^ª?PoØy'
¾?ï›"Y,}H?ƒÿ4džØ£?Kl4aùÁ?KŸF …?‡†RýÄ_˜?ƒmQkQô?îҋéá­?³ÌšCßô?kï`m¤ƒc?ŠoùðÃã?¡Kg'Ç"?²§Ÿ|½J?íæeˆ¬º?œóhø$?|Ñð>V©?€ºWYw"s?­ÿwwŽ_‡?›ŽÂq?ïµÉ\n¯¥?w%c@³û£?Ù1n"Ú´?&{Àž%¯A?'QöŽ-}?vþywÐAGN4FGL J0928.4-5256?Êãt)Ù©e¿ötmZvnÀ:4^'Ӄ À;²'Œ6ڈ@!ÈÝ:Ùâ@%"ü|?ÝTd0V4¿Yõp7©?¨#¹ P5*@^
›h¿ê·'ƒû£?﹞âƒÃD¿Ü5b¸[ü€¿èìí¼0¿Åօˆ?ª¿Ô¨˜¥}ÓjUNASNone3FGL J0928.3-5255?à/-ùý k?ËÀ˜Ìj&d?hŽ/b5ƒ?^_aZ}ú?ßp‡×Ð6?ËÓùöÀU	?؊†d;F†?ÎZ*­± ?{lâutÜ?…ú™É:º?ãƒä'!'[?Î•WÉH?æþ¿Â¼íK?°kÕHà¥?ä7{!D?ƒ
VoÌ4W?Ñ^¾É¡A?°0Ù­)5?ëq8
?œÔ­/€?{&¤ß'Ù-?gSí@ÌU.?Âît–™£Ä?#ɓh?Ý`mY…éu?ÉÃBàO`?{i-îL°?—4²É@¹?áö÷BÂ?ÉÖöÇG&Û?Ï-ÊÂË0?Æ̱xL[½?y,‹kÞì?•ö À0Z†?èjö:{É?ƾ ug~?áŠAÛT?´n †ª õ?–in\Ë@?ŠE±¼°\ð?ۅR–6?´O""&*?äUÀ´:¯©?±+á ½|?PyúáÁ?"rì™äG´?ÖiþŸL¿?±•þŘMIXED4FGL J0928.5+3916?Ú¦…1Ïþ@G:Á~ºñÀ;V›‡À<¼‰íT+Ñ@‹	ˆêË?ùÛR6-¹w?âÃ^YQªí?àyÇQc?õ
US«È@·r0É÷Z¿ë"ÿ*¿äÛibš)¿ØßüTyÕ¿ã|É´êWø¿ëáÂ]B¿ïÿž`¨·DUNASNone?ï]b??ŠR"¯%Æ?yÕÐ)p¸?rv6ێ҅?‹Ô;<RQî?"Ffë>?ï±dµryU?†p]¶£?V«w†*K?b<D!™?€ÑcÁº¯È?"*Y«ÿ?îŒÙšeœg?–ì+#ÿ•u?ˆ¬|ëÑo?"ì‡á‰"?¡G!E­±?"câ^¡¤j?ï]—éHáú?sW7fJ'?YÖ["¼òM?I])íóø??'¯%»™?rŽþ¶f?îi±+}ÿ'?žo×|žÏ?'#&ëÓØ?‰±S´,ùÐ? Ó`3Î6û?–ƒ`µ1§?îÿë¥!"?¡Áiõŝ?pÍԑ\G?'"dÂOƒ?›Ï+n:<´?žÓœ*?퇜9¡Q?Ÿ–M«õ?Ž­ÿÑ2Â]?‡ù‰VFí?¯Ú¼s•![?œ¡õt(?ÑdÙk?3üªâ¡ˆ?Y˜IT8?\~¸ÞÖ?¥Ý†$*¥?ûßCxÎéAGN4FGL J0929.3-4110¿ïô~¾»«×@Û¼ôèuÀ;¡}‹QÀ<šÐüÝ5Ñ@$œþ0'~?÷´¿û-2h?Òj«ûØ?£bt"Q†0?ÐXÅ>
+ã@džaƒ}£¿ï½ÜÿõÄ?ïÿí@_Á‡¿ÞÚf]­[¿œt‡Äã|ð¿Ý³n!EÊå¿v"쩃iUNASNone?é^ސLFˆ?Æü;Ú÷‡á?YJT–ò)?X7±ãÏ?ÊQñžW2[?Æð0¡ä^?æªö"AÕ?˫輜$?€Ãvﺩ?‹
•'>"µ?Ò#û)Mù?Ë1D¥–l?çšülïäÌ?µlÅÕP˜¹?tFGe9¢?{Yß­ï£Ò?Ðxî
V'€?µsèù.?í=0¼Ø°R?¢}®±¢³?oê¦õË:?^ö¡Øèo?µÄOÆT?¢
£.RTµ?êq¨±1?ÃÁ>óŸŽ??oá¸ÑŸÓ?o®™¶jû?Çb²z™¬Â?Þ¦ì	öE?à˜ƒ"Œ©
?Ïñb¿y
?"Ôaš
'¬?"àRÀ¶ à?Þ(UËÝø?΁¡€BÛr?çùPÐk׃?±6阁ä?'J5ˆÃù?'˜¬YÓ?ÎøØ«t?±žï‡?箂Àý?¸xÌüÒ¶â?'A_ðMSõ?}Ìv !Fl?ÐðØðœ‹?¸èÍV±þÅAGN4FGL J0930.9-3030¿à/GÃãïÿ@.&?Ýe¡EÀ:àˆÛ—À<z á!¨@ ê
½,ñ¦?ÿ…˜Æ5?ÄPƒO*`¿z¾z~À21?»5y3'K?û1Åû!sî?ÖpÁÊoû¿ä ÜïYÀ¿åk¥€Âù¿ÖÓEA¨–ã¿Þ
`¨6j¿Ó_2•~'UNASNone?ïåBºdÀ?¢¼¸C'/?Pø#3'?W$5oõšš?‰§ªøhfY?¢n‡i¯£?î"{É5NÓ?§f=‰"á ?w)ϐüx?z#0sÊ®ä?¤Ó	ˆÝJ?¦Ÿ(Û³ž?ïVIr\5W?Šmm1ê?bÔ›}6œ?P~nŽ®?'ÜN"yJ9?~°09y¸o?îDþ?i*?ƒŽÀ{Aª?wzjliçy?XΕ"‰;V?¨Àλà!†?ƒ¶—lEàù?ï þ|6 <?¤ŒÇW8'?^¡
ãœÄ?TqNÃÒ¾,?™öÉ¢_Œ?¤e=ûÆÜß?ì\6h?»Í²:zOQ?"r·e±?Ž­v†Ÿ4ò?º¸ýå–?ºä\dɝ?î¥Üْáw?'{¨òñÝO?m‡BÑÃx?`Sõ~${¾?£ÉÁVV`Ð?ÏñŽZó­?ꁮ?æA_?Ÿ{öøB½?'
ŽdÛl?{ç)›`l?Ãו2²r? ŒŸ^uC]AGN4FGL J0931.4-3559?ïŸ%¹^A@&vT´:çÀ:ÉNÀ<\ø_»Q@  x"¦s?ú¿Íui8©?Ô¹CXr?Ò¦:&l{S?÷²åB˜@l©4:D?ïËM;5Á¿æ¾‹@hî¿Ú"Ø\¢î,¿Ýzz…\!¿ÞŒy¦Ž¿íò^ç1UNASNone?ï[ìD-ν?‡›òz¶s}?\"ìeÒÃ`?Pv¾;z*š?'º(¸äk-?†—›÷ô—?ìèêî(›?¸Žþ»"[À?|˜Ùµ#qú?€ÒõÛGe?½w+
R‹?·Å¦áØW?òÀú?"•ˆnÍ2æ?{|\{ç¼?yZ'
9rp?£—µQ¦¨Û?''š6ða?î)ą38Å?žMƒü"b?s3èeˆ³¬?TõùÁutW?ªý:¥¼?*Åù6sÃ?î"ÈíÓá?Ÿö¦{Y†'?nÎñz¹'&?dAë-È&«?¥Æ¥W§'?žâ²Ü¸?çQÝÄۀ‰?È´?dfSh?ÈR¿•²?—bÓæšÉÝ?ÐnàÕÃA?È,5NQ­Ù?ìƨnQIý?£Xãˆ/v×?ˆÂ01c3Þ?'v¡Ç6r?¶²vˆ%0š?¡òØbøµÃ?ë"(¦'?š¶¬KŽN?|òùœŽ¤?n-\«»ÓÖ?ÀËÅ+ÔÖB?š4–;"v\AGN4FGL J0933.8-6232?ìB§øà…À¡2CI*ìÀ9þSW•éÀ<;<v¨Ô@­â˜»ù?ùï:µÞt?´=ÜÀ›ø*?æ&õ7O!¦@0M™gD²·?þ뮔¨n?ïçŸìš?¯GW™ˆ'?‡Æ¨½ÆA¿àµ¿äF¼¿îÚpžùÞ¿ïÿȽs"vUNASNone3FGL J0933.9-6232?sÖԑªöX?ùAõ£>?ïx;ÈO‡?­ªù†qÒ3?šCgυ?¬:ƒuC³?…}&hÁ×É?"@ˬ¾´?ê':ã‰Ze?¹ŽšëXú?Ä_BNxð?¹H«Ûª? kÄ«2v´?—žÕÃT>?êÜk"n X?°u¬IÊy`?Às`ÄTÇò?¯Ðušñ9?\ü·"·ø¡?M²ªi¶'?îü±ôÛ½?"¬BA,Àß?žš•Ê?"ë•æ·Õ?|¼x	ߤV?"Ö|ñ9µü?îߛ‹X°"?§TÊÚÁ'?œÝp•¹'?£í‰"ôR?|èyhY*H?‹TFø8À¤?ëS/ø"?À–èq:wB?ÁÊs0Vè?Àtz]5²Œ?Ÿo†ã˜òÿ?—Š)ª—o}?êóÞÚŠ¬?³ùśñ†Â?ÀB"ºÿ½1?³*¡¿,ü
?AT4›¬
î?6䕶Z¶?îÎû	îbÁ?&9ÙE¿?¢Êþ'L
s?Wšâ0PSR4FGL J0934.5+7223?±1–¡Ç¯@BÏrÅz%À:Ð.ülÎÀ<–'õ@-ÄY`Ä@Œ½}¤p?Âê¹Ç·d0¿¤òåˆZ'?Û·pú¾øy@ûow‡ ¿á†XVÙ+¿æ潤:ÝL¿êžÔ6M™ç¿ê~"àÍ4Ò¿ßÜ»­?¿¿ïNŸË6öUNASNone?ïïëWÒNí?S,Cð7¾?Ic×°}V
?DQý¿•µ?Swd·ês?K-BD$r}?ïÂw£œõ?|p0šÌ§g?T_äÁ©º?co¦'†É?y¬hÓÑíT?ufX!À5?ïTèL…Ñ?ßKçIyÀ?q|l¸¿Œ?qѐ"´?'ÛE¥?"?}i]ÒD65?ïÞBŸ"a?QªÔ8S¾ü?TõYwT?AâÞWai?gB'8á¤É?Jóø¨p‹Ì?ïæLO¹Ñ?bZøkÛt?VOÑj¾J?T'{ä0i?]Žâev6?ZL;>…ÑÛ?ïE/Ñmµ)?™Š™ðƒ?£?f'I>˜?wÇí•FZ!?"‰¼¥äàÓ?–²NÐú?îÕ
),R?ŠÑÒÀ㧳?~"–œ sô?y>3fé©á?º¹©®Á?†<ؕ±AQ?ï‡_ºr#«?uÞÍÕß8Á?tˆùù?h"lZÖï?"!_úÊ3?oìväJ†NAGN4FGL J0935.5+1152?¹t
0Ô¯@DÝ%þ—J4À;Öß3םáÀ<åCÖïe~@#^m"?ùÈÛ–ª?Ìù)a£3 ?cÕN?lì+@ÞM&yfs¿ïð®ôt±ƒ?ïìÐxR÷õ¿à5A` J¿ÖN0d¡À/¿è2D‹JK~?Õe÷áMRUNASNone?ìR\z™$?ÓK"—Àë1?¼S24¹"Ô?ÓLlÒ]§È?qžŸLgàÛ?š²f~–]?ï±òcè»H?´£q'?Vgö˜%
Þ?dSïÊt?€¶h$^0›?|ñÿ©É]œ?ïO‡vεÓ?"Ìø1ý™?ddÚa>@#?p
¶åÌLp?"'uÑîh·?'
䟢?ïù"9÷?ˆÁ¢@??p¾2cS.J?\@I¶Ró?›@üà?ˆ'˜Nªƒ?ﭓçS
ê?˜¤,ªûÈ?hHšËV°?–í£ºb²?}¾÷%««?…ûï²zp?ï2#]þ
?–»ÒK^k?dj$7?p½Ù1ç†?—8Füpæ?•T
áN–?îÓÒ0þ"_?…•ð[Œ?gï]ßnæï?jC¯V?¡Cç'­¢?‹†xNj?ìæk"xv?¤ HqE?"v9)+ÇS?~'ZfAE?¶=Ü6O±ê?¤¢]öEæAGN4FGL J0937.6-3358?éÌssó T@+&&ö¶À:Ä"À<6U¸™9"@®É"¾@tþ½	á*?Ãë"ÈÒc?–9;F8YÊ?Ò}y]9!?ýyðql©Ì?ïþ‹ Z›¿çš€'¿í.jÁ¿Ój¿ëíAÄÆn?°äÏÍÞѿɶnçi[8UNASNone?íˆç·"°H?³	¿ZWK?dê6—":?aš89P-h?³Òó;þ1?²ìÔ"XNÞ?í؂ץÏ?³röKœ¿?'A(s¤'û?ŠT8w¦æÅ?­çˆeÄÉ×?² cª	Ùg?í 	,F? "ðñîe?‹P~…‡Œþ?‰A°wV§?³í/¬0?Ÿ7›ÞÏ?ïzDºD4?r™üŸß$?RQáû"Y?E	iµ
Ÿ\?$•+bé¶?q°n'êãã?êÁñ–?Àe/ڎ+?y`=Æv}?x¾·&šþ?Ä&÷'wø?¿šõŠí?š?ë5ÁŠúD?ÃlbËH¶?Auoøµ?œà,4˜6c?Á4â"]á÷?ÂtÐï=²`?ëB<n"ü?©C?%ý¾?˜Ø)Ȇ°?'²CC'›?À‡ñÕ´–º?§JÆã(Ù¾?íø–
ëG"?–=ɍrÝ?r÷¯ŸK|"?m佺LJé?®©*`oº?"æJ#¢AGN4FGL J0938.8+5155?Ã^zÊ  	@G>L/ƒ{JÀ;Wѹ›—¡À<ãÕçþ{@Å$ʏ°¸?ÿÚáb†?ʨ3PD¼?²z5?ÙJ?éwÇ·º@ã,€±¿å
f H	"¿ä©£1ÈÏè¿å˃á÷Vc¿Ý÷µƒ¯øV¿ÎíŠG?¿ïÿ÷Ò4ÛUNASNone?ïÔ›Wý?gö¨b'í?E'øqØa?:ÐÒõ/?sW³ŠLoÓ?eÛ]»r^y?ïÐèVÚÆú?n׫)¼Jt?BòenýN¼?Idê®ë«?u-ˆ†%«?k]óÜþ?ïw\tcî×?x‹Äåâ¤?Zhyl¤­B?EàËâ¶T?ŽÛÓ±à¹?w§Y"Ðk?ïņhJ¨V?[é+Ê(˜©?IÆ~'Açš?3¹Cj9?züB÷?[†Žû2Q?ï'H†ùÑ4?yDví‰?T°V:®?Kî¸E֘?‰Ói·?€ 2™?ïq[IIAŠ?ŠóÑΈFˆ?Tcm$&%?^f¶
i/?Ž`Q̗?‰…"l²?îÜ'X^Ú?‹îïN'dj?em¾'ã?]«m¯@ô? æ¹D"¬?ŠÒâ[C$?ï=ýLOœ?|Qޛ¶'>?a«¨¢?TE
x«?–
áZxq?|qu–AGN4FGL J0940.3-7610¿ïå­ó‡qÀ1sàGÓÔÀ9Ã(xÅ
¼À<'šÈÙ"@}ðpÀÝ@:a'ÑÖø?½=߉'æL?Øü
Ý©"ã@xØ앿ð@Kœâþ?¡Ë¸$Ê׿ÃÈ{ÄÇoÁ¿Ý1{"54¿æZ—ZúøY¿ïÿëJw¿Ø\:~6UNASNone3FGL J0940.6-7609?Ä£æéGpœ?¾ÉZkJ@?éillÝo?Â*VD+Ô?¦Ù¤Kš?£P¢®æéÌ?Ö¦>ÿ«X?Ê ÒW'Ä?ád‡½_W»?Êِ'ˆ¶?ºÝ)"Í?´CBhaÂ?È$[Èp`?°§©C.¸?å…äéר&?´³=m×p€?ÁĐ›ï	?¨s Ø6?âø(& t?¦}ƒŽjf?ÌMy–«
ñ?¢S="z?ÇÑåÐÔÄ=?›IZ­nº?¯æ\¡Þºö?ª¼}%Bû?ìiXý®RJ?µƒ¤Eâ:Ý?©"€¨ku?¤ýÖ÷Fh²?ÇLOJ&P?Ã~_pAË@?æUç¡?ÈvÓ?œfí?¾¸$gFç?¸µÂ‰?±	T'¨y?¡&I*kc{?é¶	…vT?°ã/Ì·®L?À£/ß/"²?ª%`".Ç÷?Ô8Ɩ8!?§ù´ì"?Ö¹Ã}A´?®Â™HÞ8?Õ ½mfé?§*Š·lMIXED4FGL J0942.5+7620¿ï\=bX‡"@Aî‰v5çCÀ;ƒS¾ÃõŽÀ=MŽ(LO@ N
/-êõ?û]þ¸Ø#?Õ$¾!ŽE?ÝN']Šõ'@v?<Uñ¤@Ý]Ü)6/¿ïöK¶··'?ï÷
XH–r¿á³"6‹­H¿Î(ú »¿î™ð×n¿µË4*©øUNASNone?ïpí÷G}K?ƒ:؀£–*?tðëS5]?h":
žÍ?‰Á	½F†?QnòÐç??8L4?†?oæô"ˆ?lªò÷̲M?rʾ¥Ð³.?…´µ?A¨O?}¸2i'Hu?íóîǞd°?žÅˆ*x¨?'¯û¼Á•K?Žk4iY®õ?§i£mgh?™k\ï]é?ïœGãˆ??yý	ƒžôå?‰'ƒ÷r?p$AȊ?+5´á?r]e€Ì9ó?ï	5øy=?OªÝð¨Í?†Û¢¦Ô-?}'?Ÿ©.\?"šktÄØJ?‰ðÛé®?îħWzî¼?Ÿ~(»:G1?€ÊM%ؘ¼?ˆ'~ҀÜX?Ÿî|V?—¿U)¢ò¦?ìâ/ûÎˈ?£"8ü
ð?—*ô¬#-?=àÀ‡Šœ?³#Ãzò?¡SlÞŒ?í°r­,ڐ?"ä¡~
4?šhBF'Ð?Š+ÑÖQ#í?§Ä´}
??áb;AGN4FGL J0943.6+4207¿ï'ÌFÑ0ñ@H"­}|,¡À;"‰"hØ1À<"5¬En@¿KŠíÚ9@H…ªÏL?Ñë¹÷Ýò?¿Y'A'+'?ï|ˆçš®m@—¨q£±K?ïË'`—¿èŒµ( 2¿åš'bEov¿ç,	þÜix¿ïÿÿ)@k*?ï™HÁ9ñ"UNASNone?ïôÜV¾¹Ë?Qå_‡¦ZN?6¥ÿ"À?5fal"~'?P¦é3˜ÝT?NŒ<Ñz+?ï™öƒ þ ?‹ÁÞ3¤?cª#¾ßö?pöGՑÍ?"—ÖWr?…aAìé¶?ïs›Vߥ?…Šº&ْì?iµÁ]üâ?rÉο83?ŒÒýØ™?ƒ%¸—OÙ,?ïÜø"ò©¼?SDÞqÞì>?Dï{ÏÉù?-¿|ؤ–]?m˜»eÑ?QÎfÑU}¢?ïä5Ú,†Ç?maj`(-?Kðæ¾É÷?Mªl…qŠ"?dÍìD|ÕÀ?k'b½jQS?îü;áqc?©"…ŠhÛ(?l{ët‰êý?:Ùâ)U?œÞ›í1<?¨8÷Tÿo?îø-ñ߉?bMÊZ¤?q§ã	(`…?u 
Ðy?œIU²?NWŸû½¹?ïyöðó?yrž…Í?^-KzÜ5?Páø} ?÷íæ³?wþ됮ϼAGN4FGL J0944.6+5729?îÉ75:8O@F¹‰ßrïÀ;Õ09ƒ¯MÀ='¹@ ۑ×-xß?ÿœPbîâ¡?Ñè[ôrƒ?'ÅiV/âq?¶¥ŒÁïÏ?ý§gıË?çD ¾{ü%¿ãøÃ*Œ›"¿åϙ/çNX¿Þ§¨ìMñ¿à¡¿}ƒäQ¿Þ73ÞSÝÎUNASNone?ïÚk'žÅ?dÏ#Ý}?=|öÍ/?0àlP}Ì?pò}52ÛU?c´°jþ;?ïp¶Æûýg?Ž¸Â·q²$?i7õè$Ÿ?pè»Ö|?"Q•Á?‰Þ)	œ]…?ïO`GéM·?"@ê%'+x?`‡[Iîß?Y<\'ø8?"û¦Ð4<?ƒÇ®ÇªO?ïg€0¼á?wH7ŒiFt?i"ˆUÐrC?PwÌ9.î?ÓýØ-_&?w;F:?ï¸Uô.?v	1o}?Eÿ":ö?;‰Ïî¡ît?€ŠÁ4Ì9!?u"<úü?î©·u'kg?£x,\`p\?sså'Üà?|ŽW,rá?¢öñŒ?¡ÚX‹
c?ÿüá#?*¹`ðl?gì<È»?bCŠ~~¢&?£G¦ýmD?Uwúº%=?íäÕhbü
?–s˜òã^u?€¢û(m?s©Ýó´lØ?­Šùzf	?—5ÆDú.PAGN4FGL J0944.7-5124?ë¾÷!F?övaÍ
àÀ:xÙÔLgÀ<»få@ Ú¤.™p?ý{ÛB±U?ћ)Q2!»?ÏîƒUà\L@S_2•?ý%'6¥®{¿âšÆÀCQŽ?ïÅ2¤—ú]?Òë@Ö3ÿ¿ØîŒÛE5"¿âù́'²Ì¿à¹ë^2eXUNASNone?êT#uGw/?µÏF§«Áj?{c~2í‰w?qû›vþa?ÅÔV8ÆÅø?µG*V÷¦?Ý ¥×ÀpÉ?ЅþC‰¹õ?¦bý?"Óyñ$ô@?àïœû_t?ÐD¼áêŽ?ëFÍ)Á?¦!ôN?'̈6ùD?†ôÄLE‰ê?À¡±É™Å?¤"‹óLC?éà	ëï°Z?šm÷"ð™M?š—M¥TÅ?{‡$O×5?Å,îšÚ!?™AiŒ¡?åE؍†w?À¼zš%?éʨÜí?ƒ¥>Aôáþ?Ôu"ß×}?¿žóíh?Óò›-mv{?ÉÑ>Ã×}?˜¹ßkDx?¥5ÇÊõÖ?å@êZ@,/?ÉGk9	?åL,£÷ì`?³¿>tâ?¡
ŒÍ¥?'ŒÒÙfü?ÓEg6ߪ?²»Ps^<?å	¦¦Ľ?¬¸N§¸(A? ¹[ë^y?Žºÿ^W²?ÓՇ6ü§—?¬4mñ¥=JMIXED4FGL J0947.0-3548¿ß××C›ý@+ˆ7q†UÀ9øúÒ¶À<óähÊÅ@FjpŒ/#@\0LÎå¬?Å=ê†Ç?áÇV +à@ìxc¾ì9@œI1wF^?ï«<ú\R¿à±%q©ˆ¿éñ&³ÈïÈ¿ïÿÿ" 5•?ïʧ߭z¿¦:ÌbLXýUNASNone?îÁÎcr8?µ§@×M¾¬?¥GNØÐó?±Rú´ø¬?•Y½œ¿O?šo‹i…I?ìúņ÷?À!Á?šÆZ+•f ?¨{¡:f?±}kHâí­?¹Èc$(\?çoÔ<>?±ˆH…™¡?­4+*Ñ?ª÷æüœö?¿)‰Èmº?¦Í¢þ¥Àw?ï+l¦CÕ?‹ˆJ®þDd?dL%®IƒÉ?eøö(ªˆ?˜ùYåÒí?‰Oaé´L?ìKÀO?»nÞ&ˆÍ;?´À'Á^È?¶;,ë@?¥Ê~'¤?¥#樣Ï?èà?@B÷?̳pÛ4n?µ¾Û‡¥?Âq	^Û?Á }?-ä?ÝUn½?äêàgÎ	R?³½(Ö« i?DZœžöi˜?¯WÊîÛ}Z?Ä¢áÁÑq!?ª˜ð+•'Ë?ëohí÷Œ5?µHŸ)7 ?•Fý.XFØ?ž×¯ä:¥ä?¿2ùD­Œž?²yÊÇ9AGN4FGL J0947.8-4234?í¨ÓsZ@ þØôù;ÁÀ:[=~HÀ;ý57ð1V@¶ P¢@°cûRV?ËOÿÇ é?Åëq¾cÒ?úÂ(]í@Σ'•¿Û¡ßyw»¿Ã³œd¥-¿å]&¡ª_:¿äÞ?:þ¿éð9¹_2¿ïÿØ}ZÙUNASNone?ê#L…ê,?µoq/ µ?Øµ¥tá?pEG¾ð?ÅuLí2aÁ?´Ž-ÊérË?í{à(Ò»?²là¿M&\?s'p"&g?tÀP›+›?¶‰©ö(ÓÃ?±Øóa6%×?ìì÷·S‹:?â½úÌåK?ŒO`RŠ˜H?'ÐMe²?µV;€F¨?š•îù¤DŽ?îlÒZî?x´®&¨8(?¡ÆC-ª?ZéJc%ì/?¤ÊnXºö?v}]d!ù?áFŠE"²û?À*Û};?¢ŒŒØ>?"®…JYQ?Û!Yô_…C?¿ñƒÕ%û?è£c(栀?Ä»l°µó?‹a8Rw‰3?–í	5çK1?˼_׫øí?ÃThôw?çQÚæÀê?°yÛøFŸ¸?¥À:!¡ÖÎ?"í»+{(?ÍKrjz%?­…P·R'?ìˆhCá+?"V31h\?"ö›Zíj?vtìŠÞ

?ºæç%œ$?'Á¡ÔU~AGN4FGL J0948.0-3859¿ÓüŒ-râ@&y*Qã!£À:¶¾(Å(À<£hOt²@›"j8-@A³ÿvmE?ג¥^žÆÕ?êÅÂíOú@'ë¾íç?þ õ;5?ç÷X[á¨&¿ÝñÆ@ì"M¿ìþ£^"_ô¿ïÿ'ãñ?ïø¼ßï¿@¿ïûÂ-·sUNASNone?êLÎJë?Ãí˜Z€?'‡L{‹?'ä¥VrDÄ?ÅUÞXæK#?ÂE›,?ê}[‡²ˆË?Ç,*°ãs?¢7pjÝTÁ?«2ZAÖ>Z?Á|µÆ~‡£?ÄB(E»Ã]?éKËÄÓÈÙ?«R·°kµ?³ç¢|q^ ?¡y_Z\²?ÀÜÿ®æ Ë?¥j컈4u?íjOɹ>r?¢»š‰¥þ?{
ÉS4?}E˜âû½o?²ü¥#šÌ»?¡Ž-Õ¦:<?ç´ÑòE¸?'nP<>°Ñ?©ýAb·?©	Ä׎[s?Ê­ph?Pð?Ãnþ˜5Z?ä—òãÖ?ÐÞÒvƒ"?¿}ø[úZW?Å쾆ÛH]?ÍäÐ	ÿC~?ÊÏøWŒ?åi£àDxÖ?±íy~fÐS?Àؖ.«6?©°Y@öÜ?ɀÚPCs?ªƒó Š{?ån¸Íïë?Á(Àú—Ç?¢ukM	?¨\Åjñ?ÒÓì#²À:?À4æu¯~AGN4FGL J0949.8+7551¿î61yc‡ÿ@B?ÖbwÄ]À:îJÔ9¨˜À<ÚµŠè@ø™Iè^?ÿj~…A?έ©MÙ?Ó¦¿òɶ˜@¡/à˜[¬@‹¸Þ6¿ë¸Á>#Q¿ÉÿÓµI¿àÃ.ô	Q¸¿ä ¶© ¿èae`,¨¿ïÿõƒ¥;ŽUNASNone3FGL J0950.4+7550?ï˜öÆeÕ?yÚ¡Ó 7Q?p¯ék®Å?e=t-fÒ?¼¢œÈY=?s2"iîu?ïw2G_K?†£»]C?oåúkyŸK?qô¼D‡K?Š9ÚøqI?¸•oË?ïcÚ‹&?M-îk?€ERâ©l›?~ò&PP?—PæLz¬ï?‡ËŒN¬?ï	IúÂJà?t©¹²Ë½+?†À.²ë?d's'ôt‰?"v½‡Æ™"?o,Ý|d?îþv9\ÿ?öu
ð©3?…˜E(¦0?€—d˜€sê?•eB';?‡ $bµ×¾?î]f¿ý†?£ƒ-¦C?…U™p'?‹¥˜ÅGB?¤Ñ¹*4…8?žŠop€d¢?îb=c?˜ªK®Ú?îgÚ¸Pr?‰&®*™?¦r¨EÝC?'¤¦ûÈ[ü?íŸoçg?'Ax©³£?–,^B}?~ï¹¾Tg?ªòòÞ%Ý?Œ¦7Wr<9AGN4FGL J0951.8-3711¿éØ?ì¡uÓ@*-À3aVÀ:µž·æ‹»À<:îí‰@AÜ¢òô@¯BÇ$í?Ö9íAat9?î~;¹ÿk@>l`{jÚ@3ô–#î¿ìÏj¡^‰ù?¢Âæo
Nã¿ìà=lòò¿çí?3¶?¿ïüBK?ïęAÚëÉUNASNone2FGL J0952.7-3717?æm&Ú	vK?ǚrõŸ?¹RÙýÈÿI?Á—×uzÞ÷?É¡÷˜õ§.?ÁâÙ1<Á…?èüÕ2½(?ŐýOß~?À\ÈfûPˆ?¿ÌZv™"?·_Æj™7/?¶|NèÂâî?è"3Ö?°W´¡ü¢O?¼Àv›EsÛ?¥¸ü°F,«?Áãåî?§XZÂÀų?ê¦IR¯Oc?¦êÁjÉ?·˜œK;r? 	t%ŸT?³5ì0q?–"ˆýXõ~?âÅ&w…j?Ëp@fÄÒz?¹ùþ´%Œ?º[ĝƒ§?Ó÷3bØè9?ÈMƒŸ?ßá5òL°?Ï¢6Ó	I?ÕdùVó
?ͧ~xoÂ?Ås¡ø¸¸ï?ÀuØyƯ?ä?\ÆC_•?´4%&¤0V?ÆZEÂh+?¯Ì£Æ¾÷¿?ȨG$ŠVŽ?®Ü6Š8?ßîž_7YD?º~6'›µ?Ñÿ–Ö͛?¹x
<Zw?Ì#—6	s¿?±¯rƒ\ÈAGN4FGL J0953.6-1509?ê×I"¼K(@=šO—íÇïÀ9Î,UÉ`1À<ˆ¢Ù´;Ü@"²U}5
?ú»	 :2+?ºžolIP?å(U{\˜@%%"1zÌ@9RIMü¸¿í<Lû[V?æžÞ&'d¿ÉMgfìs¿æ	s˜Ôx¿î"žã…uö¿ïûÌßÂðUNASNone3FGL J0953.7-1510?›vFЖR_?š¾ú.ãJñ?îSé¶?¢ÜçVxÎ?éÐ<â?'Š ø›?­ªÆ¡;XÙ?ºŸËç
"'?ì~›PuZÂ?À]VæIS9?ªk"V"?¦i"óŽ?¶=°e%-=?¦|(•¿R?ë+Ëǂú¶?¬OÍ¿-Ub?°cñ^U	˜?Ÿ$l•b?°‡£¹ M§?"©î"€Ä?ìp'Áv>?œÓÊó²?­y¶œÑ?Ñb;gæ?—hxr)(?"†WäŸâ?îÐð¥ïé2?Íö3·÷?Œò厅V{?‹÷´ZyÃò?"A+ïG %? E
ږáo?î"–cs?¯	C%½«|?¤=ð¡IX'?¥´9m‰ñ0?§g´Ý&h?ž}
0öË?ìÂí »r™?¥ÏÈkôWÇ?¬QÆ@G—?ší8DmÞ?š®þ"jì¸?…·­þ@èG?ìè¡øôÚ? ùüʅ8¨?²0"€?›…0Žº®ÂPSR4FGL J0955.8-4106?ép ¾*al@%ì|•|ÔÀ:@\78{rÀ;¼$·om@ÙÜ»W@z[ñ?ÑsÓÜí?â*8ÅC@Þ¦c¬wÃ@]!)ÆM¿Õ§ÕÜëÓοàøi"®U¾¿êû/—@ú¿ïÿò(¦è7?Ѩ©ï?çjNRsjUNASNone?íÌ5×k?¹xhï[+Æ?{æbcç÷?'
ü´¤=‰?¯¿ãU0{K?¹áaUñ©?í]¤~4Ž?¹üüÀZxœ?–q³Ú4*?¢×k:¥\4?¯%‡ÃR?µ_Õ¢?êL¤ê?©ƒ›²KâÅ?®nîRâ?œÇîiö*ú?ÀN±´Ÿ.?¤a¸?îÜç/,F
?5âÁÔìÄ?bÐlŒÑ?]ŒÉ»‹?¡†O}?ŽÖ̖KOl?ìkeeyEU?ºbàV䵙?"¼)4®gÅ?——é7³íÐ?·uʆ.Th?¸X0S~?é·9h4$}?ÉV°¬ÁЬ?±ZÒCx2"?¼Eà+p¾{?Àu±>ô(ÿ?µû´ã?å¹õbJÖq?±'°Ã·?½Fùÿ§?¦Ö]Ï{ï3?ÊtêzT&j?ªÌÒِ±g?êÁ­Ï(<?³°öþ?‰ë_›,Qÿ?‹Z›¬ï6Ú?ÃZ'ʿί?²""H>5¯AGN4FGL J0957.3-3851?ëóÏ^ç0@(ú˧2ßPÀ:sö•3À;í┵.K@¬Þ½e&@—s\.Ë?Ñ+^×{Ò?Ó
©`áí?ü%F
¦L?ö—‰çtî¿¿ÞqOÎtm¿ä[Ò>%Õ}¿í»ñ³6"Ò¿â'¢;(Êú¿î»Oag#%¿ïÞú̺XVUNASNone?ꚢi]"?À%°(@*?©×xLlë?¯
IéGÊ?¾¡øð¹ˆ?ºMbçßU?ê¤Ü­q›?¿öèi¶R?±®´:E%m?¯O€°£þ?¹*k—s:?¸$âðe?è¤e	;Šg?®|Õàê"?²³›òfÌ?¡¢>©•ˆ?ĝ⺰ý?¨`?^Ne?éFæRýr? 'NQ´¸
?¶êï>wº?–ւ©?¾ÝÞWŽ²5?—Z*l/ì?ço¦ ï?Ä`R6iÛ?¿sèG­?½\ÕæHkK?‡sz(á?»Èh•{ä?âÌ8îž6?Ëù4|çå¶?Ê~¬èD¼6?Æ<ˆÿ9þÌ?ÊPpâ&Œm?ËwL½Û?äU<ûçu?´{XC?Á¦³ÜC•à?®
eÔ»Ç?Î÷/ÌÌL?°UþuÁl?àfÆà"š?±,<"ëÀ?˧˜Æñýš?¯g}"Ý ?Ñ^¥ÜaÙþ?­Gΰ-®AGN4FGL J0957.6-3051?ì6ÞãÈd@2µ,'¦77À;(Òü'¶vÀ<šˆÉg½~@nןc³@9lÅûø4?ցùje?ì)KRä©b@
´¡\Üyé@re"C¡À¿æR:Ê×)G¿Ö™}j¿æt5ýö¿ïû©žõN ?éŸ@¤Šä?çÂ)óUNASNone?îwŸ@€?­µeð"Q?¥
Þ,%?•,ñ§Wd?¡&bk…ö?¦ªƒøw¿b?î˜àÚ?´¢y‰{5Î?™ËZ§ƒvž?§±Qß*N[?¢0Ä®p@Z?ªêÃo
aÉ?éâãm*ÙP?««x‰q€?´ÇFNћÕ?¡°ŠöäYy?¼!žJÙB&?¤™w¸WÑ¡?ï}|¥du?µÕGˆÆ?c‹êâ"è?e,֗»?‹ÖfZª?~­DHe¾±?íƒå{«ƒ7?²òMÌÒÜ$?–_ã"8"J?šEGfúi?¬'¶"¢f?®ñLë¸l»?êU†Fxå?ÈX3
ښQ?¸NRLÂÀ?ÃøiOò?µ{ë,:?µ¥d{ÍQ?æ%]æÕ?³%½·Ñ«?Á¾EÓýKM?«vMºÆ?ÅÙ$´jU^?¬˜×³ÍÐÂ?ìÆp…VÊ?°­º@‹¾î?"g	Ïa§?œ³/d>}?´ò¹aß8Í?ª›.c"‹±AGN4FGL J0957.6-5208?²ÑÇQp‡"@ɤ^ïÀ:€<_+߂À;Ï _Š@è°XÍÌ|@X¢t3¯?Êm§"n>ø?±´p	¨Ja?æͳaÁ»ø@Xœsé†Â¿î;Ɵâ?ïöÌD琝¿áãñâ0a¿é+ñUBQ´¿å"†ŸìÄå¿à—|ÞÍÖ7UNASNone?îõmé=÷?–ÂßÓy?N0â{£ó/?E(yŠ÷:˜? 0]ã,'?–‹Aós±?ëê@OÄn?À£:N§Ð?hÏi*­%?ztô2Ž•?¿í·
Dä?¿)Z_z—~?íc¸ÙrD? üç"Ì?;Šsw£%?z€]0?à?µ
pëãXù? /9óN"L? þ8'?z"þ·íuñ?g$t¬Q?Ká÷Y"é?£ÓÆÎÞª?yÐ\Y^In?ínr¤ëº×?¨¢mpÏS˜?f§o±7Ž?aÍw´Åَ?³×/^3ßM?¨XâaŒ÷p?çǝŒ>V?Ç.Äs>f?ƒ÷àó?¡kîáU¸?Ï°Pâ'ÿ?ÆSbcއñ?éFkdZ¦?°ð=ÓÖ?'44­4?È?…í™j;m?ÈÁ¼# /?°Z¯|é?ìpv_?–¹Úy*/Ì?yëG'Ü?h#§b¤¡Ë?¹ö¥Æ"?–UHÞu~£AGN4FGL J0957.7-3510¿ïá_ŧ-@.Οð˯–À:svð!fÀ<(˯–[!@Rqé&t´@!Mryš ?×Ëq'úä?áƧ"=çÂ@	o!öÊÍ?ÿÅäÆh¯—?ïú²]à°Ú¿æˆ(Øîn¿êædþ²M¿ï†Ä);
?æûÎRÞÊ¿¹ŒÔ_":UNASNone?ïdŸ=ŒA[?°½»ýe©¥?ƒÙ`™‡?£ˆåýgÍ?'ÿ%Aßo¦?¥ÊºÈ;¹?ìžðãyÙØ?¾Õf­oK?¡Î(Ӛ?«ÎÄɞ?²|УK=?¸‡X÷®pî?ëP$ú ¬?¦â" "0d?¬œ>¹žþ¦?·|Ò?|?·0¸Ñ	 Ò?¡ž?'R‡¾?î‰ä~Þò?"²[‡e9–?zýÝ!ó?w¨ƒ
Êi?¤øS,Z£?'mµ~™¼?î«1Ž²$?§ƒka¦LÖ?"¯ÏÚÖø?£¶DŽ?ŠÓù.-$?h±I'¶?æïÕqƒr?Î0ÐJŽL<?ÀCúÎ	Z?Åùsg€`?Ä'h±'ªY?Ã\Ñ@"²¿?èf랖zù?¯'\Q©Z?¸S€ýã½?¥©.Ž¾Q?ÂZ'Å'"??¦à…øc9Ç?çَt«R?½5^h|?¦=¤Öû?ªI4Íù-å?Ë
bÄñ69?¹Ÿ°èsOAGN4FGL J0958.6-0522?æ, s—@=@BŒ>§¼À;"žõ#-,À<›w3=D.@ØZ°O¾"@²¾‰¬½?Â9q{BkŠ¿±"Žg·IX?í1išÐ?ù͙Ëî€|?Åû`ž{U·¿â;}^ûc
¿ìúþ£ßm¹?ÙÈuO7u¸¿â¥ýzïð8w?Ò~UNASNone?ï}çÁ'(ƒ?‹<óõ\mQ?W#ñèãHW?Oˆð¶Ø?¡'j"?Šn:Üzç?ïµÇ3Áà?€Ô[€g#?[M?'k,?kþ²¥=?~¤Lâ
"?xƒæíòV?î¯÷µ6`Ã?"­6{ßkØ?mÀ7»²6?p$ôFZw±?£$ƒ…ð•5?""!¬¼ÐÅ?ïDôö:?}«Ž÷Š?xøo'	Ö&?iÓº2Q<?'0%¡J$?xÉk%¡?ïUa]ûÂ?Ø.k'Š@?hÄ8sJå«?aÁ˜µô¼&?';MN‹€?ŒZáÌ.ƒ?ï"ôDǏ?œàjs]½?sµ^'R'Y?‹›ofþq?–´ÉøEÇ?"UՄ_f?î l§ÑžK?š¾Ëç¦k/?t¸Oô~Qs?sì7\Ö?«b+(­ ?™ÙÙä	þ?íftÑ«•? ©‡Wµ?œÒ±N}LÃ?–Ì0¨pJ?«/f™ëR?˜hNmØ<ñAGN4FGL J0959.1-6441¿ïâœU>S€ÀâDÀú0³À:˜8±ø50À<§÷*ni@Á¥"Ò@-IÿþR?Ðô«£‡Y%?Î"øþYà?ý·}°/@¹‡!m¿Ývz"ð¿ç—ØÏ9Ž—¿çW\¨w'î¿ÞГásÍØ¿ïÿýF\I¿ïƒY¡\ºUNASNone?ì "¼ºÓH?¯]F¿ón¤?ô·=°?"nÊkO+?»‹€@?¬/ˆ5û?è*L‹¸Ÿ2?À.Ü{/e?{½»´¹í	?DŸÎ.O2?ÎxßòÎ?¿¹Í/Œú>?íHa:ò3?›òÍX(?
á,·Á?…ʳwN0´?±Þ Ñï'í?˜I~':?íÅȞaKí?‡ª¥Ïj³h?''Œ¯':?bòs¦š?¯"Þä ?†(­qˆpŒ?æ#FG¦Ìw?À,Wï!­Ç?ž"">7Uÿ?'ñSQ.ó?ÑÑ1M!hR?¿_$ 4˜?àQÚ¬ù?ÇêµÈyV?‡J)Fó?'¡ÆO4e?ß
ýMâÑ?ǵ)mÇ	?é–á®[H?ª¸Ót~è?¤Ñl&–X!?•XUºCH¯?ÆUInÅÚ?§>¨æ¡[Æ?êRU.IƒF?¡ôŽÐÆ_(?"oº%"ßØ?€&!EØ£Ü?ÄH´¨+-? ö ïh÷ôAGN4FGL J0959.1+5719?ÕßÆcú@G¥"À%À;b,µj°À<"φ»p"@‡Ž6¼@ÂzÞÃo?Ã)2(q8R¿¶ï.vŠ÷?ô`­¤éXõ@6á¿Î¼?ÁqËýTª¿êB±(+˜¿çc˜UÌ»¿ëõÖEòR˜?ØÓ P—ó¿ïþ±¶ÆÑ
UNASNone?îã9Lk­<?À¹ë­§\j?ŒÊ{£_L3?³
џ'W?•3˜Ÿ"äi?´­+5§›?ïp\áØM?' Rxe?nÕúȆŠª?xí¡Û"ÙK?Œ**ql7?‰ß‡–`ç?îí¿›-dß?ŽYrä®S?t9ïQsÝ?wžÄåAtª?9¾€c%?‹¼¼ÀWvô?ï¾äû¨é?hò8±•@?8ùøÆÀ}?3vª®'?ÂmX·?gg(ײR|?îݍÙê9?ª,œd?|)¥4ì<?‰I{ý…?CÛxÁo½?¥åfGmãï?îÈ¥pµ?¦ó?"ÙG?x‹dQØ´?"Sá©}½E? mb?K€˜?¡C­[›ÆÀ?î
'{¢–K?–Ö½ç$é?€v7þí°ñ?~©zRЉ?«úGO?"Þ½ov?îÏ;~.ˆ?'–-ä'Y?_Õï=>"°?aòinúxÈ?¢
˜ É"[?'˜|ÓvAGN4FGL J1001.3-2040?ſtP{1h@:ê7&úÆÀ;LÇ+£ùÀ<½oe©P@ ŠUŽ¡™?õL«	-¦+?áÀá?µ"?ã…ߨq£±@tœŠâ?ôÜþ(º¿ëì&ďç?ÐݧESÇ'?ïÅTӖëi¿¸ÜÐ{)Ñ¿æ—IÈ î"¿ïÿÿ" 5•UNASNone?ïÐÐv
Ú`?p™Øšg $?YrVB"šf?U'œ;á^?q;/Q4y§?k"K¶hº?îªÏÿ[7?¤½`¯S{c?'¶Ãü
?šËŒFO
½?™•ëk?•ghaͬ?îli߆| ?˜¿HöV–?…ǧà3zä?"t¡ã'Ø?£Çx»I?•s›ûk??ël³sàM?¡;Ée×MÄ?›:bªÙ­½?‰‹¯rµ.?½ÍYº†y+? Ù)‡¦T?ï§Ö¡j{ý?€ñ•«Û^?m™«HÖÑ
?oùÔ]^Ç?}GÙ¸4´?xàòŠ€?ìnáûdK?ºñâ°ä¹Ó?§$Œ\‡Nð?³ˆÐ77?°ö¬ä÷¬?¬±¿¡³Fþ?í"b'ßTÔ? @æË·µ?Š[ùJæˆ?†®®rTy?°lF^ºõ?Dº¿åü?éVN•±¤ö?²:õŒ?"TÊ\°?"Ši_pý?ÈC;Úõk?±ø¬b׸$AGN4FGL J1002.3-2810?ëŸ\¼!7@5k»ƒÏ,ùÀ:әt°¬À<<íÜçÍ@n݃S\@!]³9}Ð?çÓÌ@
>?íU/<-­¸@¦ó|cþ­?ó-ƒ«ñŠò?ïö%÷
ø¿ß¸ç¨eÝ¿ìuL}‡\¿áó{jª¿ï÷dP±¿ïüK_ÏÉVUNASNone3FGL J1002.0-2837?é²9Ø,Á?ÉTÉÜ(?À"¿Úmk¶?dž…•«£\?±d±ŒRÔÑ?´±
‡°º?Ù°,iP·º?ÔwSÚ¯?ß³`«¢–Ô?ÔÌ5gß?ºqˬ2ÅÇ?¹yÊ…¢?èéáPp
?®L9?kï ?´"DF;â?¡o¥ÂVX%?ÂX›«\?¨P‰–}k¢?¹9ºUPê?«Ñä3§¿{?ê£Fª?¶" >/ƒ?±¬¬Â"‡?©Ud塞»?ç†=òØX?É&éP¡¬?Ì<ÅSíÏ?ÈÈÜ/ôÂé?¦©ïcpU?ª]Ý+ÄÈÕ?Ǎ`N'
?Ι¬%¯´[?æªÅ=·E§?Ò#•_?»u÷´?º¹³³~О?æ14cÙn?±"Ÿ•Ï8!?½Yßß
?¦D¶¯"D?Ȏ?¦ç"€?¬¸±ÛD¢?›ÂœÕà³?œêø4nAˆ?êxŸ£kKö?Çúb1Mæ?Â¥-×(ÆH?ÅånË 
žMIXED4FGL J1003.7+7049?½½úü#ì2@D4cŠ	À;Ä5LèæßÀ<ÝrÐ×ôH@ ñc='Ó@
&ˆó?ÄÐR¾=èÄ¿·é¥´¦?퉎;Tj@³sŠfK¿åV'""F¿ç5:	Iú¿çú+	™ö¿êø¥˜«]?ÊÃgÉ<õT¿à•½ÀƒUNASNone?î	ã©2=ë?ÈAd"a…?NÕu'±õÃ?eÚÑçx¨"?®æo•w§?È7¶
ú–?ïq¸vÿeÑ?'}¯)åó?k~0´Š* ?töa¬|z?Œ²V""I?‹ç/ƒ1k?îì&`UÄò?È
ê@…i?côèraE¼?fga¸R©ˆ?Ÿü–íVõ?¥Õ¦µíÕ?ï«Ì{]\?sWE3(\ÿ?8´6Ž{Æ?1…Rç@ñ?"G?{¶DÎ?s\gòÉì?í'ëÿåJi?À¡Oæ-x?`Ky‡t¹?tKÚ8Ž?³h%£}ž?ÀÛj|ÿ
?îÒî-*ì¤?¦¡ö!iD?r:ª=.Hc?ƒÁbÞãúã? ‰ÇæõG3?¤ljEõÖÒ?îêšÝM?—†5¬i-?mð—'ßx?i³á-~Ö±?­U'…È/?—pEÂ€?îOi
õ@M?›ßÒ¸ôþš?^¿=Æ˳?`¾tMdvÊ?ªue£A?›ëø©LÿˆAGN4FGL J1004.6-5215¿èê)T@5+Z÷[À;"÷8±!vÀ<‰E=÷²T@î­94?ÿ÷i=±;w?×RaA
'c?éÚÝfx@¥ߙX@|´>
§¤¿ä9Œ~($?ïøٛhÞ¿Ô¹+ºîÓÞ¿Ýq׳°œ¿ïÖèå1G¡¿ïWîÕSUNASNone3FGL J1003.7-5215?ã?yƦ©3?ë¬ãð¢6?±Ã+rÑW?¢ÄՂ_¦?Õ@[§hÅ?ÂÙÓʱ®R?×ZÈè*?ɁÁGÕÏ?ÆŽƒØ"?¼22j‡?Ý×Þ0Õé_?ÆqD¬¾u­?ê;•ÿu~?ª9;4.fã?®tÙk¢­˜?š·‹—ð®?¾èãKòÐJ?¤:h'Ü*?æ±vÍSX?¥F
Á¹½3?Äï´ß¬^©?¡»L>ý)?ÀJoì2Sö?šÕÚu?Ü©bí酞?³KÐÂ?»`y¹¼È?¬#·GÝíº?Ü~~£Ò‹0?Ã,ŸÙ'Es?ŤÒ4C}?Ânóp5Ù?Іºx{*²?ǂúóÉh?âSn65éh?ɒ·}/U®?å+TŲ¯É?´/%J{?ºxÂDļ?¥Ûb†šÔÑ?Îð…í?±w.ºÇt?ÝK]ě?²ŠbyY΢?ÑÒ8BÞï?³íÔÖT¸?Ðâ×iø…ý?°Pjc+MIXED4FGL J1004.8-5250¿î?Ä!hÂ@—a_–iÀ;9
ÏÌ[ŽÀ<X·Q:…@$Þ.ŒÛE6?ø†Ì7{—P?Ňϗ­[B¿·¸ËŸ6wÇ?ù¡cýÖZ@JÒ1e©¿ïÿ˜f"²Ð?ïÿõ^'¿¸œmŒ?¿éf è¿äj&¯—1à?Ê[å™w_ÞUNASNone?Ýë<%Â~¸?Ðæ³u/N?WÏû‹?WKdy¥ý?àþßå¿s.?лٛ£p?ѨîÏ?ÏA?Õä'?•]£º¨à?¡ÆŸ(}6\?æv8›Iix?Ï-¶?8?æqC1¶Žû?³ÿéxIÕÆ?yzè#xö?|aÎõƔ?Ò·û«²v?´)>oàÇ?ã!ø2¯]?¾¦Anp‡8?†Òۗ†h?~"ã¯eQt?Ùxò§tE?¿'æçnþ?àk¼A—Ø'?Ϫ«²a?r"ÕbÝÐ?qº"©7?ÞÞ8'—QH?Ï®'"ÉG?Ç÷Nh÷Bö?ÆPq:2‰s?"}§2¤ç?£ú]¿?éf?,:Æz?ÆñšÂ8Ÿ.?æîí4»u?°P¨&3Í5?ŽL²«Ñd?‡ëü/>q?Ñ5³1+'K?°… ð?ÑçÕÍÛ@?À\¶ÇY?"p¬K´´?˜ã&ÒèõÁ?æp;q"?Á›Öc›ÓMIXED4FGL J1005.5-5708c?äTÂÅÀq¨¿ór˜Ù€9vÀ8ùáy,;ÈÀ:s™LlÀ@<½J£½@7­eÿ8Z?Ê»˜Ý\#?ã·¦±.@ö£ð4±@ðbF¿íÖ®b~zY?é0ðÎ3Õ¿çñûûŽ8¿ìài·ª¿ïþ݋`ñ²¿ãÙ}'ÕUNASNone,?ÎeÚÇ®¢?Ä¥U|?È<,Ð?Ä-4°O­?âx}Âoô?Í1þóÄ?½ét3"¾$?ºƒ7
5ì?ÓοF¸‡W?'
¬ÄwF?â[qÖ1$?ÁäçUO?Ñ#ÑËÕ?²[6[§?É+}"?­bÅ,{{O?á#™Q—™²?´\¿±vÔ?«OÎÖY–ß?ˆ^g`Ù«û?ÓÁP֏Í?§î:…	?äjsêfk?¨ß2GSe?ºàŸÛ…ªØ?µ¢Ù)¢?ÍUéÁz3?Ƌ	dhñl?åaŠì?Ë2Í]<?£x}lß?ª
q`HØ?×1äcÂG8?ǟ¨^Oãå?ã/¶®Ê¦?ÆÑͬ_ˆÀ?ÅÄÏî-+?ªžý³SçÏ?ÊéëÄp?±k‰´Ú×?ãÔhÄSpY?µ\zé"?‰É&.zØ2?pa¹5ÈI?؍ßÓ 	F?³"i Æm9?ãQë}š"?³¦h½R'OTHER4FGL J1006.9-2806?îѯ¨#Ë@6!>‰¨‹À;=Õ¾
iÀ<m7Žâ†r@ÅñÞ&Ò@™þ†ƒ<`?Ì™<§{/?'ÑŠægAq?̃ÛÂ3@‹µ`£¯?ïåe¶™…?ì†e	o‹¿ì£é~´;¿Ø%}}":7¿Üøe-×)¿ïþ´ -UNASNone?ïG¸,p%?ŽDóK§ùM?_6¸ú	'e?Yt. ?•Žàíô?ŒÎ?Gü^"?ï¨ñ6Ÿµy?†b§/¨eð?YÏ©®Lø?cV²ìâN?'‰ÑI$-?ƒÓógUK¤?îÍ<7$Ã?'È7Š?xæ§Ñ
¯?|¬¢?ògž? g®¾X'?bût…,?ï@H›?vSê`¦?uV2 ¦ä?`
òòÔZú?'¡`jøs?s€ÊB<f<?î×0øè«ó?•és̀v³?qoﬖ»Š?nÉ)
oF5? ^òy¬ä?"O3t¦º?ï&[w±"³?Ÿé¾5Šoh?nÐD‰(`?'6!B!?—ZˆyƁ?šÈ¢…Kdõ?î
@ZŸD?˜ó,:¤`?ƒ"&`ÖöB?'´È¢-Ue?ªMÒaZd°?–=[¥úa?í×Í\rO[?"®TÈ¡rk?×5ng_â?"5ÆÅÇ?«
\ÜeKR?'$<ñ*/AGN4FGL J1007.8-4514?ΞÅÄVô@!>—Ðk½¾À;^(Àª'À<p‹â÷±}@!ö¤Q-š?þù²©5?ÆÛK•ª¡ª¿²ˆœFG7!?óõ«é'v@vä;ÿ4©¿Ó¬ž"Í¿áw™:¿ê®ßa$F¿ïÏüE±?îüwµCCL¿ÒP|VUNASNone?íáEƒlÜ?ª…Êl»¹+?P Î@'&ñ?SqfþÉj‰?°µ"œÜþ?ªP
&Æÿˆ?ä)*¤Õs ?ÍegÎErÑ?Ž<5ÇTkQ?–ڄ›‡?Ö»É5óF?̶›•Î?ì…e*ã>º?¢±I˜ã+Ø?m" ¦^?}ô_þåC?¹Ýý`^Ì?¢`LÒÑ?ï?s«&?‰Ù¡Yr?$=§÷Ĥ?&Kÿ£9¹f?—ö–<w?‰
xYM?ë}øìîÞÎ?º}°s¿")?alï©[¨?_¢LÞbç?ÁÂhæ¡?ºT—鸍G?ÜîxªF÷?Í%ÒþÑ=?`)À«œÊ? …«]åI?á|‡u³>?Ì\÷TVd?éSm?«=•ÀN¹?‰n_‰Frþ?"Ë[V¿‰«?Êì¸?«°›»HE?ëö³bîaÈ?²E",9iº?M€ëŠîJ?Wÿî^8y?À±‰>F{?²B­=íÈMIXED4FGL J1008.2-1000?åzñ+¤Ò@AߥÁƍÀ:7äÞ;ŠÀ<PP¿54•@ãá5E@)ªIë?Ãb'Z/÷??µvÄ­n§?ëýdQµ@gõ†Tmk¿Ø³D›:ƒŠ¿èfœK›à¿í|KÀrÌP¿åï`«;'¿ï÷¶O²Å»¿îʇB'UNASNone?ïÁ«E€¢?‰³"ÓÇà?h•ï{½?qZÅ	ë?rße¥Ô?"¼yæD?ïŠõm?ŽZP_g9b?p—4wÉj¹?}½2'±Ãf?"÷
=9ª?'mM"nï_?¬Á?—¿ðökº`?"ªmEü'?"Û.4·;?¢<ãÌrÓÀ?"ç,©¿.?ïx¦¯×Ÿ?kíÞ¿ìÔ?|½Ï7™÷ô?e+_yj)?t…Ýck´Ø?Xo<jÀÆ`?ïŽÕÃüà?ˆVÆK®s(?€­NK¢HÊ?€U(y…›?w:Áðª"?z×æIã0a?îŽ,Wha?«"QÈü\?‡ýT÷Jœ(?—H¸Ùå^ö?¡èûÚëï?¤Vsuµ½%?í£‰}Óъ? 	‰ÃB?"ç´û6üó?%¶mš?«Ó¢"³ê?˜à­ô'V?îÈ4¹4€?V–1&µï?˜¼å¿†?‹èŒ')Ä?Œy-ÿÿ?w±dr.iAGN4FGL J1009.5-0034¿ï.­+`›@Eß;dZÀ; ¯7'À<ˆ©í¤³©@Þ@ÌùÃP@RpEy‹?ÔÅ$'n|?Ô­ÎÚÄU?û¦y–ÄÓ@
›Ž¹¿ïÿŸ‡ð#ê?ïõ}€3l¿Ý ó*.§³¿ç¦Æþ¬˜Ð¿ãmZ@¾61¿íÚï9ßßUNASNone?ï!ÞL&M?Ý©3­'?q؝6Æ^?e›iUÏ?—'\™Ä?[™Ö¥?ïlل"ù?ˆŸÜa'Ö²?pÃÏ}J;_?r?.µ[?Œ—áÛ:?'5¥IÂ>?îg£???—wí	?Ž9þ2Þ?4?‰êÞøÌď?¡÷L†¤?'ð$F¯‡…?`+?ƒi0\G‹P?/î†æ ¡?rPåp§?¦ÎlÙóC?€!þrŒB?î{*ýúI?˜'×þ}?~Úµ ç½Ó?rN^.tâŸ?¤qù|	9/?•ð)ÜÿÄ?î?Û³?¤ÖnSs.F?†´§ð}È?&˜jüjx?¦bT&%Œ4? ~¬f!ˆk?ígEn©­? G€›f?•¿JÎÈ_?â<(?®¬¸ù­?™ÐiñR–?ëš%~¶X?›[^šúî?™±9²'(?ˆFÎýpÜ÷?¼Â'¾œt?™eæw™ÛAGN4FGL J1010.0+1416¿ìPÚÁŠ¬õ@I*û~ÿ—À:ëG‰+MÀ<eÝãu…¾@¬¸§{Úl@L®ì?Á¸#G'Ëw¿»wۃÉΖ?ø†!Ðý?ö…ÓÉÁ)«?éÛÁÝ/›¿èî÷ßËF¿íŽÌKD¿Ç³A¶X¿Ñ(}ãǐ¿ïÿ^º z^UNASNone?îï7TnÛð?²ÆQfš«Í?~)Ô fo{?¡%ÇM§•À?šŽ h×	0?¯£µŽX"?ï>3."°?—8ŠyÚÑ6?{êùÍOÃQ?Š2YQQ—§?'>Û̳¼?ŒÉ³ÚæՇ?íÚÆÉí8A?žÛ@¯Qû?'ÞæXMÅ?4®¬}o?©Ç#îU?™¬ÿ"MÄ?ïFjå?fS*NO?t·J¹rŒ?gèFÌ?'
§2eV?|½ÞV'Îö?î­x‰Ëé?¨íãœÜ?ŽÐÛ:¨çM?–µ,žÎʙ?šôÃNsK?£gr	o±?íò"Œà+?´š¢r°J?" c¨¿þè?® Û	)2?§ßbaÛ?¤ìLCûWz?ìôâÍëñ?¢,AœÎ?™¥9[.?•¦£ú7íl?±ï›Kñ+?^Š—ê?í;v3õ?¤ª´w€?šzùD,³?–Ä¿ߐ?°‡žÐLy? SVۂ<ôAGN4FGL J1011.4-5729c?ïýÁìôàg¿ð¡ÒM?MôÀ8ÁÚWÏÊ®À:Fá$r¦@kŸ~Šõg@b¡ Ï?͹§@¡/æ?ÖK2»"@÷ñsuB¢@|{ðȀ?ÛªcÇOµ?ÈTZŠ»x¿ç½¾a¥"¿é¿*þ~ð¿ïò-DéN?îK®UNASNone,?ÔƜ¹ý?Æ2"õ†Ý?« jY•;Ÿ?·iò?=¦«?ãêªý³ä7?ÇÎͅ%æ'?Ì­øôütc?Âüíh›i?¶'zlxfS?®kn ã?æ2túÜ]?¢úWAt?ÎÙ|‡ÃŒ?±Š6==s	?Â7¦ÓqŠ:?© iËÙYc?ã»Ñ쬏?³¾j0xØT?¿I…Á0Ȇ?œG§â?¾ÒE»(¾?œðÖ«î'á?èF"ÿ"×?¤Ê–§Ô?Â>ãό‰€?¿#ã+€Y?œ†õØ'ׇ?¢2¿O,?êŒ]@"?Àý¤†¿¸?²*ǶnH?²Ö݉íÜ?½¸õ"|?º"H¤ÎE?êˆSÝ3?À9Û×4bf?ÂÎVB_~ž?¨@Ñå?ÁU›]>Ÿ?©l]'Ï¢?æ÷—(R?°¿¹Ähl~?žße¿Þ?…bØ$_Sú?Âð%Œ¬v@?©kq1(i?êLýўæ?©–éîŸ0OTHER4FGL J1014.6+6126¿¤ëŽðþmI@Gsý'w>%À<#§ÝÿúøÀ=k-àãÛ@Ãf0‹Ž@'9¾g¯<?Þ:Gĺ¯"?æ"äÁ5>ü@	~?íëÑT›ä¿ïO±^p‡?ï·l]¡E࿺;ùÖEF†¿åèQ'¿è&ch¿ðUNASNone?ëôƒˆò=±?Ãqåí"?º;
©7'‰?ÁXø<šÃ™?˜ƒdC¹w·?¥4ƒ¬|³?ãwß×ãΓ?Ц×cöí?Ó`2¬?ρ$…f?¶Àµ:<šn?®Ø`J_Î?éÄ!3Æ?®)†ø\f–?»ŠÆ‹ܸ?¨cAm˜Ô?¶T jÖþù?¢Œ"Ôñz?Ü8^vÐ?²íë(%<?ß¹î̄†?³h«œј?°6Êõå¨n?¡`ÝÕ!žÐ?ês&Eí}¥?ÄÌ{®¢g?ÂK]æ)?ÕƆÈ5?Ÿ@HPdx?¢8;êar?×/hN"-³?Òó‡Ãü?àòÏ.À¢?Ó] ë® x?Á}d(bc'?¸ÔRR¸?ç'Ý@Ʌ?°æÉô†ò?ÂâêƒÁì?®βŒ!?½¬ö$¬T)?¤÷=«›³?ËMÄ8ԇ×?³ÃÀ¼ùQ?ä™ì/
&?ÁP3³¿=?ÂJ‹ÝT?¸7_
#/àMIXED4FGL J1015.1-6353¿åP4†'!À.ÝÎ|Ð5À:yªÜ·ü[À<(íA°¤@z¤®Ë"ù?üü|¢èÍ´?ÓTª|?ì?Ü9ïô8@—€)†?ú}YÊ¡¤U¿Ô(ðd+£¿äõiøØÄ¿àä›ök+È¿ß,qãr*À¿ç'vµiù¿ïþÎÝHEUNASNone?ì-Üæº?¯´"8½ug?'™aZï®?zÇ·4mC?¼DfÖø?®b	)\`L?á3YÛWmê?Â''F¥< ?"ëÿÁ6ƒ¯?'j†[¤?ÜJŒM"??ÁÄp
j\ü?êd˜íÿ?ª'{]±q?£zÌÆ^÷ò?"þ}2«"ñ?ÁŽéG?¦c5­2?æòc5ôŒ? Š±'?¥o@¹¸Ü?†,¯ão°?ÎÚ«Xo?ž~ÊTZFß?æ›?½ôÜz?¼wñ¢?œ‰­4Î`?"¥Gyp—?чéBú&?»KÑ(•å?ÐDêÉ?­?Ák¿!àÈ?œŽ;­Û9? ¸¡¶bkõ?çk­UÁ±?ÁšÃ\­øC?åÆéÖ?_?³"\Â?®«‰¢~æ'?œ	°†YƧ?ÒøV?±Ð•!Û_?Þº?ȗß?¬ §FSÂ?¬£%¸»É?–æ–i¼ÆÀ?ݱ‰	©w?¬5ҔŸÐ9MIXED4FGL J1015.5-6030¿àÈCë^ª¨À	¾±›îÞpÀ8¼o´ëÀ;{'¾Šë@ÁIÿþR@Ž¼g#ü?¹µ¥ÿ-?ÄÂÇû¬´)@¨É¸EV?ö`õ˜ó×S¿ÁO¿Ez³z¿ã'Ž½É¿êw$>£©¾¿ëèU{\˜¿àÑÉ oâ¿è½Êeê?¤UNASNone3FGL J1016.5-6034?㣵&gó¯?Émtò	6#?¤Yƒ/8?­¸!y´?Ö-eN
?ÈnIÔàAŸ?Û~éãfŸÐ?Êˎ‹jú?³ÕRý.è–?±àWw˜åU?ߋÁ]ò"J?ÇýáïÁø?ߥâ{x†?³¤7­@j~?º4pëP?¥ 
y/á?ÙÍèëL¦?²ÌØÐmŸ?Øö–ñYÛ$?©Û'Ôþkù?ÃÎâ!ƒït?¢šKjI?Ý!÷ýä-"?©^'c¿d|?Þ×÷ImÉ?ƚž‰9òa?¹
†ï¾j?³æ_×N?Úä¦û#n¼?Æ\üÌ* Ì?ċÉy}'É?ÃøÕ~]d?ÀRuKUÐ?ÀõÂÜ«_?æÈpZ
Æ?Ææí÷â¶?Ø!%'"ì?±ºò9˜Òõ?ÀcʁæA
?§Â"ëÔÓ@?߬‹™{¼?²$Û%Cö?Â(‹·Ù¡?¢4O%Ͳ
?ÐØã¶É*V?´ÎÃêµqæ?ã	ˆA­tm?´1˜>ÕÈMIXED4FGL J1016.1-4247?¥íÆrŽ¿€@&ùþɟãÀ:H¿è+ÎÀ<L 鄓x@ °æãÏGÑ?ûtyŸ(NÔ?ÂNÔ8üËÃ?Ä+S?î¦@—ԝ{¦@&ÎEÃö?æúÂG¸¦¿ê1s	â×Ñ?æ±x7I¿ÛX'}ÆV¿Ö8\½Æ¿å@W©4APUNASNone3FGL J1016.6-4244?ï)›×ü?SÖ²Lð~?jq`">‡?]áÉ,²ý?—`tx¼™?¿K+Ò…?í¼²m…i?²ÿ·æË?u6ø9š?{4"äX™œ?°Æý%A|?²FüŽ]x?îÞ¥¾QE(?Œô.3ƶE?nzK&ð0á?j,š–…o? -ÿiB"í?‹o3‡áM?í¬{O,8?‰à¤…çÓ?z¦ën§î;?e¾Ž]µÄœ?°ñ¸‡¤Z?ˆ¿*%W"]?íê/´¬";?¢'ìÓ¾´?"ÿøF˜Ø¹?y2,!lôa?¬ŸL#)? º‹ã•¿"?ë	Nã	q?ÂWöê‹,L?†dSIz³«?'â Ú¼µº?Ât?"Å?Á¾÷¢
†{?íAyKè®!?ŸÜÃkÎOò?~ï3?Ϥ?wÐJ¹?Z?´Blސõ?žàÿ§?ê‹|ÃӇ…?£'½0?ˆìÎðŸ'?ïékó?ÄC@ÞãŒ?£H7T¿šÁAGN4FGL J1016.2-5729c?ëìõVƒÅG¿åًâvØ$À9[ãU¥NÀ:iÀ¬-@:šœxò@?ޚTª|?È<¨èA€?·6ј–?ò¸ ?¦=@í±GC¿ïø§¡o%þ?ïïNlta¿çU%`â˜ç¿æÓ{rg%©¿æÕ²^·po¿é¯?¨¢UNASNone8?ğÛ¶ð?¹ž×_ç‹?‹=ý'x±?'aâ:a'?êkCRî˜?»«J	þ?×`S¾TJ@?Ë%Ê íWÔ?"ÍÊ7Û?˜£Ch>ë"?ã±n
…Ñ!?Ê:æ¡mÆ?Ð38Þæ!T?°Ÿ.µÜ?¾z¯;Êäô?«o+Aã³?ä
©?³Ý&º€¤?ئ…VoE?®é³?'O?™dܱBîí?zõüÎ̜?âᖌ/4?®ñ­\éÛ?¿ó5õ¸ÜÞ?´¦ìÜØJ¿?†bïäSý?‡Â•R!Î?ë¨
·"p?¶xۀf9?Ê\î~´w'?ÃfPÁä?¡1@»m:&?­Êðg|S?èU°TàÆÄ?Ã:ïÇú?ĔUό½
?ª,D?½óQ­e?®aØóWÃ9?ç€V|Žq?´
|ZÄr?ÈDÔsô™?«|CŸvš?¡uâ¥2l?Š¶Äk¸ƒ?è×lÎèäc?¬úH½Ö\:OTHER4FGL J1017.4+5956?ïáM‡ó)@HQüLYÀ;¥
ÒÁÙÀ=
GR¤è'@¡Y¢<U@´'òÜ+?É -à
?˜K­A[õ?ÐG¯Áú
ó@a+´ä¤?éuv¿ê–ºö6¿Øv'•p?¿èi?Ñ&N¿î)gØVmË?éÒܱF^‰UNASNone?ïlCÎ>šx?Œí0µªq?^(Äk;¤§?Uc˜~(÷?"ùééÒ½?‹'ÿ''Ó?ïwQI?q$ÿjŽ&?gqܖ
oM?lό•†+×?ŒO6':??‰q°5V<ç?îj	à˜J~?—Çd-&(ß?ƒ'-ry!.?"\ª­Â‹J?¤~֙±Ö?•K·Èà'W?ﰍ²M?hxÞóÉÆr?c¢™ôcŽÎ?N­­ö'êd?}è*
×o?f¡ )›þ?î<AúÖ?¦Sɨ·^?qLJ5?i!yG¢ª‡?ªÞs%W?¥¦Âɧ?îšmy?©çºF´Ûš?r¾¨]ˆò"?~#!,â?¤ªñÀ("?¨Þg¤œ€?ìø¼†Ðá|?¥N€2Âg?ˆqîëì³Ù?…ÚçWª›?µ+Ýëv§?£àG–×`?îá´^ýø?Š¯è5jg?{²Ý7'Y?r&'i‰ä?œñ¢¹
Ê ?‰–Ê›LtAGN4FGL J1018.1-4051¿æ"VÌё@*"4çhZÀ:¢ï	7·&À<;EM*Ë@I'VT'@E®æ1ø¡?˂ºZ•?ÍÔ`)‹i«?ÿñõ*¹çî@ØÌàBö?îH`A]ò¿ätcI{t¿ç‡§ßW"æ¿èa3¡˜¶¿êÐ0Áhë¿ïÿØÝý ÓUNASNone?îovWË?­p.»Ì—?J]o'w ?«Ÿf¯ƒÞ?¡¶$Ö+Ï?–û4[Â(?í¾Ë-v–ñ?°è‰3x?¾ëó	¡?‰ÊlëÓ³?¬í®Q‰ ?¬¶LyG˜?î‡=™hœL?'`Vo9?ˆË	ÕÌ
?'Aÿ0ўä?¡‹3§Ü¯A?Œýý¶é?í¥ê"x?eùî;Üù?'n¦W÷?kÿ²øò7?¬wL"†¤?~'"d
»û?ê¼FeG¶?´Ç@˜ÏÙÂ? 2éUQg½?"uÜK ?Á,°ç?³'}c×5Ÿ?ê&D¡´_?ÂÈ*UþÍ?¦O½r/Ö?ªE¨'t÷¿?ÁÒþو%?À°}Ì3ŸÀ?ì+÷{æÅ
?£ëÈ4?¡—¯e‡?"ãA¬"^|?µÔlnP¤?žE1–Lž?éW°@­¢Ä?›"á	"q?§g׆mÿ?ˆU1Û{X"?ÄÇI]ço?˜1ÂÄ
AGN4FGL J1018.1-2705¿Â…âÚ¢šÂ@8u#Ä*fÜÀ:hõZŠÀ<8a|ÚQ@ɓ¨=÷1@˜ºvˆó?ĪՁ&[4?Á½¿~/°È?ú¡Üär@!͕I¨À?ïý:óñÔÄ¿åvv½Ì¿çmâ0·-¿éŸÚÚ®7¿ä:ˆA'O¿ïúp &'UNASNone?ïŽõא¨¸?¡°Þ	Ú '?hlº«É…?gÖÕ~?†;îåó±µ?¡ ¢'à™"?ï;QØ9èY?š¨ùŽä?zØðpºì?xÅI Zòv?'߈áòk?‡$¡ùN/ð?ï&®Ø›5?ƒ…ñ枚^?vùð@¼`?s\zd€?•k¨çâŸ>?…izä?îŽ)ìb"J?xwé·rß?‰_×bS?g†ÑóT¯Z? ½‰GmÑ
?sØ»ÅtÞ?îÔêMÄ·ˆ?¢…0
ö?"ñŠ\¿èq?'˜Â­YØ?šéñ™~É?–±—ùA±?íä旁Äï?§©îŠé{Ð?'yۇQwÕ?—`÷€ni.?¨ô¨Á§@%? $*•m?íÖ ,½š¢?™|˜iß:å?'¬õR8B?ˆÅÐ\¸ãm?ª&ºY »?"1€K?ë¯Û­eSl?""Í2Ãä«?¢yؚF£å?†Û¯3vßa?¹D6GD/?•<"æÙAGN4FGL J1018.2+0145¿ã°/²š@F³jçÕfÏÀ;$©Á/À<±²•"@]ï-õ±?þŸô╋î?ٔ"â-1<?ïýwå?@dÞÁÁÖÐ?úØ]å
‹Y?ëÿDïY­¿ç˜>»&²¿Ê7Üæ"¿ê'äÏ"£¿ïý!(n´?ïòH¢0AUNASNone?íÇÓµ•L?ª‡zñÙcÃ?"Pÿ´%˜?"H´¯®¿?©Úµ1"fn?¥µ'àóßÜ?åZðÐHh‹?Ιj"ôC^?ÎßØ3CŠ€?ËÜÈöÜô@?·hÉÉ[§?²3?¾ùþÉ?êŒ#æÓÍâ?©óCBÅ®h?±…®C¡tÂ? 'l¿;¬¹?º2‰««?£%sçŠ<?àӃ 3?²®'ð7H?Ð+Ta×
"?±f-®gp¢?ÏJ	-Ñ–?«¬U-	÷›?êåÎ|€À?¸ä 'Ë
?ªq&'¾?©'"'s¶?»'ÖÆd—ž?´.þÏ"å?ØƔn·mÀ?ÒÌyü×h?ÜA2€Áí‡?Ók"Ú"K?Åðr!
Ir?ÂB¦\g?çÉiRÔä?±@¾Œ?µRBRÙîS?£™
Ùa¤˜?Æ19‹~¡?«ìÓžúU?Ì"M4»Ù?±<i.®v?ԁ[#+?½G ®~á?ÝmÄä þé?»ÍÜ{ҚMIXED4FGL J1018.3-0703?ÑføÌHÝ@CÌÅûø3ƒÀ:¥·gà¹êÀ<c@ìF@@\ mf@"V^±f??Ðyu'
5ô?ǟxÖ«rà?÷‰÷/væ@­9ó–»?炙›L!A¿å)
`EË¿ß
œ¦"Sß¿ïÌdAÈø,?ãèߢ'fŸ¿ïýŒó˜épUNASNone?ï,כÕ*Œ?¸,+¬?r<{ÔT?"ƒ'_?•ß½h¡l0?´zã6uÑÌ?ï¡V‡ EE?‰bïʎë&?b±Âã^ó?q•Ä
e¸?'þø"?'ŸS&t‡1?î€*UF¶ü?•[Om6ËT?~Â+:îÂ?ܞF¿''?¤%@"ê?"ð÷€4ð?ïÓÀgÊЯ?a³Ÿúè±2?1@d]R×?,…-ZÉ?uÅΆV`?a%…ˆ{°?îõ¢+ìöl? 3Vïz÷˜?rOÏÞ;•p?u€û3Û®K?œ·ÆƒÇ<?])YTU?ï<±u)á?™¢Qûª™?i¸Ç,‡ñô?}ø¯Ž)w=?•2¸d
®?"øÙêlp?ìö3•{Q?¡>Ì;Ôغ?'yyçÃ5Y?‰‰üϑ&?³°Ø~r&?œÌîrÉR?ïe×îŒ?"4ÇtS¨?Ip'ì'ƒ?L~MUD–?'y}¦f4&?ƒ½±<ª«'AGN4FGL J1018.4+2210?ÜRi?@Kƒ9Ÿ]þ¹À<jQÎ_À=[Ëñr@%+¶ü?ñ¥"}c?çd#Ë·#?ã,ù'þtæ?õáÄüó0?þD!!㪊¿îëç?ï2Ôy±¿îéDg8~¿ïš|¨"2?ïÙ|s%'?À"v>öŠáUNASNone?ìL¯§ç©â?Àl½>J¤¥?f«âá}?o:ƒð¡#?¼é…a ¦K?ÀNÊ.s3?î 畦<?·|NN?'µ¯'l´è?¥'@þ¤•‰?¤–·ÞÝÁ?°ÍÈâìÑ?êÍiY­<Ü?«èÝ;Íì?™ž%x=ù?"Ïwðÿ?Á–•êHÄÑ?ª‡NFí¡Å?ì©NXÜ?²ßJñÉd?\üpʪæ?eáW$ª[j?ºCSÉ£?²Ú¤Õ ©$?íCI|1?´çЃA'»?ƒÛˆ	Jí¿?‰_¶a
ò?±vÓwà?³‰c¼·¿?ì9"êq3°?ÃE§×t-?¢úYê~¥?·ö*/9º?´¶—ÿ#-?¹þ6¸×U?ëJ¤jUY?©2³â|)?Ÿ¦à*'?•–Z.{'¼?¾Bó*ë¢6?¦âË«~bJ?ã­IçL!c?ȶ¿'·U?vŽ]ôM?•Þ½e&?ØK)ø)¥s?ÈîcF1£ÍAGN4FGL J1019.3+5625¿Ü"HocÛ@I
¿cíÀ<©.bÀ=5óþj@!
"´ÛŒ?÷ÚWdjã¤?ÝEÈa-A'?àt†_U% @)!ÌÙb@ÊO*Š˜¿àÜäÝdʅ¿ïýE¥ü~k?ï¸7îƒ×¿ÑÏÜâ¹_¿âA¿Þ&çJ¿ï·a–5UNASNone?ïÆ*d`/s?Žyìµ]_ü?T2p(¨³ò?[ÃQ¥At?wÞ1·ÿ©x?‹|ØóÀN?ï¢Û:‰úÑ?"îœÙ©¤á?^áë&Ýïõ?gѽy×<?ƒlôœkŸ?€Ñ¼æª3?îáÌkÜ?™­-Žó<?"çœÑ?";<e7Ç?£5½µÞ?—68F#˜?ïj¾y;Äì?r«`Gg?VÓð•ÇWŽ?E
)P‰Äà?':ñÌG
?qtî«?Ch"?…Z?h3w?g"A¶»Î?g\_B‡Æ?‡pž³à"?'ûPÁ°?îõE]éP?¡³ØÔÕËG?q¸´"Å?'Ÿç&@b?i*+›¼?ž¾m¼Ûç?ísg˜‹¨?£­õ}7f³?|NM='#?'ÿ£ÂÐR?²ŸãŽ}a?£MAôŽ,?îr˜jçÌÐ?'ü"s¸K›?]‰ž[×?Xôë±i?§ê1KLe¦?'º«ü·dõAGN4FGL J1020.4-5314?Ζb¿@	•,ß?–À:Ž¸c­OÀ<Jr&Ü
@âhgs@½ºŠ&_?Îÿ*˜>?â_t¤íŠ²@)M<É´ê?þhà;"€«¿ïÿÞý¦ßR?ïÿÞý¦ßR¿Ú)ÜÈBy¿éˆÛÜ4I¿én"‡êD­¿ïóóí£*UNASNone?ع2ú[ÙÎ?ÇK'ä©?àPNí¬sï?Ʌn`Ó ñ?º˜¼­x|F?²ÐQ–!?½œ)< €z?·ÏÊÙÝ g?ÙRùL1²?Ç,™Ë'Û?߈¢¸žŽî?Äö?nÍ4ž?ތÂj77?²¡rfÈ?Òeë*ʝ·?°‰º2f:º?ΤÓÖΦ?¬l÷("È@?Òð&ÀÖkÔ?§×Ý–Ç?âÓ"Ž?¯ÌêR9uÒ?ÁÐfL¶?«Ô–Ë­Ô?ŧ>r×bþ?¼%XæÕ?ä¶ÁÑ#Ò ?ǙðªU1=?Ç}ºJ¿?¿Ååõ4As?¥7"íä?G?§òw"&·&?ހ_¶ÉÖ"?ʀF¡Ïóô?Þد«Ì"?ÉF¶¤'£C?Ôg¹©š?²ŽZÔÀiÆ?Ù_u£g›?¶èÓŠ®c?Ò9¢ïaU?²=MÔ6]?´OgWŽBŠ?–…Q_¯m?çõä§E:?¶gíòXÄà?ƹ·#ö³?µsÖP)FMIXED4FGL J1021.8-6308¿ßW`0À}VlôÀ;+Ò/]À<'Ÿu{­ @!P-"áô§@¢>ü•u?Ä7A"Z¿³bÎ~€?óÔ*tGÐy?÷Ûb¯L´9?éJZÌÕ0I¿åÈÂ&*·¿è|"Ý¿äå¶rî4&¿ãžÅý0B? ý#à7–UNASNone?ìzã‰V?´ijÜb'?h§£Dؕ?–slÙÿ¬?¾‹{§HâP?³R¶‡ñ8'?áìra?ǂð•~×Ì?ˆcÐśN?'`‡F‰;?Ûdؔ"®£?ÆýtIþÑ­?í~Ë–Z?žŸæ™QQ?yywð¼h?p½"rzw¿?µôr'@´ò?çƒ"
&?æï¥ì–Ê?®È¯ð²«?Ó‰.±Q?yæí¨ñ£?Ñ#4k;b?¯0›?æÁ•W{Î?ÁçðêŽT?nˆ*~G?aÉo¶r?Ò?Äû`ø­?Àø`Žáæ?ÑS,=ÜÀœ?ÅÛ&	‡œ?ŽT`Ýîæ±?œ/ghóH1?æÝ]ޜG?Ä䣜ìy)?éCˆíh½s?ª§
Õ¾~?ˆ%g{`ßÄ?yÝ­á²?Éo…Òpz?©œN3L…*?Öò§Z€?¶t~ þ?¡:jokô?˜¬BcˆØ°?ã¬`NH?·÷KaKv*MIXED4FGL J1026.2-5731¿·GÇãۑt?–Òi!ŠFôÀ9éû±¼¦À;olŸe‹@Jê½£@|<âž4?Ŗ•BÇк?æ¢~ù˜@±À"š^»@qܗð÷ú¿Þž±{¸ˆ¿é֑Ýµñ¿¾Nx^
¢E¿ç±×JÕ¿í%óìÌG¿ïÿÚÁ,/´UNASNone3FGL J1026.2-5730?uQ†8'ñ?‡Rß(¢"?èˆù	Š?Åœ4ÿf'?Ï7Oé]`?Äáþ¼wÙÅ?˜x†,2¯?œ§4çÝ,=?ÕÒí*îÊ?ÂÁý]ZÆm?ä®RX÷î?–z:}n?µŒ6Dëw?¢s—‰@}k?áE0U°²?µDÈÝA³?Ø'͝W>?´& ʔ¨?¤»À›ñK?GªFa¥?Ø1ÙìÅæ?®
ÅÓIÄ?⥷ZØ?­ÙŽMÌkÈ?‹&çn`É?³å$V}cy?çªÌLÒÊ?ĖR²n ?Ï¢`TJýL?Ã)ÝFöG?ƒþ¥+Wût?‰S§i]^!?ÕH—ä7Íw?dz*D!B?å¹y*Z¿?Çp$5ˆ?¦è†m–&5?–æúâA¦?âTäàX´'?¹Ù&¿ù?Øy%qdØX?¸Uø&ý Ñ?'¾½%Ëþ?h"qf—?ۥꇕ,š?¶yî[^2?ááÿÁc.›?¶NŠH5&gMIXED4FGL J1027.4-6324?Å	3O¸¤øÀ'…‹Å›€À;¬7æ÷~À<š¿£ï]ñ@$»D;Îã?öœY~÷W?Ñ^˜¼¤áv?§C.d'®?Ó5ëŸJÞv@Ta#0†±¿ï†'_8u?äv†ºŸ¤¿ìÏ¡}éÑ?Ûq¸ß¯þ`¿á^@'—FÙ?›"£Q
AUNASNone?è/#©¨Z}?ÆcŠ¢8'?Ld]¯ò[¡?Gõôÿ/?Ï'û!Z)?Æ^´D¯v??èçìýˆ›?ɓw<Õ?ekŽodz?v5òoPÁ?ϊ²@­"?ÉZhgƒ®?ç~6e(	?µ¤Ÿ¯æÀœ?j¼H|[?iÚA'bî?ÐÏs¼vy•?µ·áŒB06?î¸Æ¡uÂ5?"xb¨›ß?ZRñ•â0ˆ?Q'Ó4A9?£ þ_8l%?'þæ+kß9?ê"{1ú? ÄæÏWl?[r硌ôš?W³"öV…á?Ǹ'â3n?¼ev|^?ààžÇ'—?ϨÔÕ,?k[ÉCÊ=?ˆzTÇçè?Þ5dÞ?ÏfÃI|†õ?èÇu™xü?­v¶çO?xPB Nö?sšçïe~?Ì/`4X?­JKuñµ?룞Îç?°å–Ï~	?vB3fâk?wþ*J¨Ü?À¿s.1&û?°Ýώg;AGN4FGL J1028.1-3550¿íLÉ*gø@2‰)ˆ†À;;$ŲÀ<qÀã/@àåK@ðO‹XŽ?ÀŒDœg)Z¿²ˆLj;Ýý?õ$#–=â@t#I†0Ü?ïÿ¯þ_ìпïmªÈ–g?Ò×#gäè¿îx™¿YFÃ?Ò£ƒþ&â¿ÀU\ã°¿UNASNone?í¥]
2~¿?Çú‹Caöâ?U˜j~Ú?a‰ùfÔb}?²€ù4•Ñ?Çü0jg8?î¸mԄŸ?ªòz×Ɵ?}Eå.nۆ?…ìšõ®? Ðqʂ ª?¨à¨ÀLÃ?íqké™Gu?¡	eïÈû1?‰™»çòùú?ŠÈ«0Õ?±Ai5Éq–?ŸP*ãùý?ïY(½ZáD?}-¿\×?B5DdØ\3?@"öª¯úN?"I>4—Ù?|±ÍjžÜ?êßÔ´?¯Viþ}GI?h£§R>?jÓêŽV×ì?¦ZFâ+rŽ?®Õ³åÅù?íuä"©Î?¹3³²cÃ?†vRðýS‰?—ü†ÐsˆS?±'Û¿<?·cûü/ÿ?ìÙÙ5÷ð?¥brÙïӖ?3âš9^?ê—1683?»¤<_׬?¤tûM
ù?í[w?Q¤?¢i¸Ã?b­Ø,Í?gÅø=X?´"À—®^­?¢Zˆˆ`rmAGN4FGL J1028.4-1539¿Ú=ë?­·@Au~ºñ6À;úÀoÇÀ<vc¹ã»ý@ˆ<[Ðá/@À_@˜?ÎYßð@¿¨0ïáú±b?èu ޜØé@'
_Ä¿è!¡ÇåÝ¿ÎôK@ññ¿ì(Àéi¼¿"¿¹úô9¿çoP…S'x¿ÝݖH¬AUNASNone?ï˜tCQl? ß;#šù?TWòuÌâ|?w9Usf_t?‡Wðìažž?œ<Uh3½i?ïÏ""ö?p=
+&"R?GB,R÷Ò=?Méö9Ú:?uŽ)0ur¯?ké=Œ£ ?ï+zŸ$ë>?Œ(œ°Ôš?jš¾ì{?q¿§‰îê?—=i	\^Ë?Š?€ª|™B?ï'dµÐö—?kûUñ«?Yn&"`j?Da×w])?ˆ9
ªÇñ?iUЁ	B[?ïu¶}ªû—?‡NFqïՒ?^ñ:Nâ:?VÏ؁ç?ŽÎâ}m{õ?…óª;?w?ï{ØÙJ‰'?‰å¶3Ëaý?VôHÜþ¡C?`×@»/?Ž+@ "€?‡ú©*»}`?îšJMDñ?" Iªü•?q—²<ÍÆ?rV'ÕÊ,Í?¤(dÚ‡Q?'S;-¶C?	pJ?/¶£?xà0bæƒ?k9aKMŸ?¤³òë'`?‹@š1Á"tAGN4FGL J1029.4-0828¿êyßofÀ(@D@ۜsh­À;!KeY -À<ŽL%r€P@6;ƒd@á#=ò©Ö?¿Ïq—ÇÝO¿·Ž†@ ?õ»‡*+M@ÅCýÛ¸x¿ì!E_…¡•¿ã2¸ÿ»a•¿âc×dÖC¿á@÷A¿á¿¾¥пÄO1ÁnìUNASNone?ïʖÆDaH?r+ä<Y'c?Ob'•)À?AÏ@Ó7?vÐЀ¡&1?pô&u8%?ï¨E'–5Ñ?}ò'4#?X*W*ù"?]k9±gñ ?'ék++®®?y"Z)<€?ïuî˔n?W?á#<?]ðƒû튩?OΒñMÙ.?ŽÆ<¢¹! ?~G«fPç?ïu!½ós³?o‰"ÀÄ?YÐ5Û®ºÝ?CÉ4'P.´?}‰ÁÕåà?n𢊜
>?ï•ÏA"•–?òk‹Ìú?cØÈ.[¡?["4R­úâ?…Æ9y#ƒ?~%°›ð2A?ïs'm}?—ۓÌì{?fhê»"gø?q¾ޕLÝ?™ÄrM^ß]?•
¶œœŸ?îåeRºC?ŽÕÏy…?j%y"_C?aH‰6ð	? SEJ×?ŠPF¿W?íõ-û!/6?'p­À¶?vôì&Å?iªVͶ0?­Î'É7ZÏ?'‹Ê°ŒAGN4FGL J1029.9+7335¿ïŠ4ûpŠh@Cü¥aMø±À;–|tÅ¥À<ö)¢¹ @ §N}ça?úÌ
Jݐ?ß.M»tµµ?Õÿ™¾, ó?üLØç&?ûÏ?Ž
oE?ïû³ûð¿ì\šP}F¿áÃ9¦û¿µ;—Ÿˆ4Ü¿á"ÀĀοïÿÂÃ^UNASNone?ï:Œ.ˆ:?–ÇW!aêû?f"4:HÁ?`Êzs¡ÕÙ?•øgôõ¤¡?•¨±yV¥?ï
€!´–Ü?š´ãô¶?ŒÑ}jGÊ?€t¬sg¶?–lÇo€?–dÊ_(<\?îdÈk‹‹±?˜¡½;Q?€œCd#++?'3Õõ1qD?¥Œhrsÿ›?–¢,sKd?íÛ·_ÁöI?Œæ±ÉgòÀ?†5I°D£@?s>#é̇b?¬·7œõœ?Šv´Öû"£?îšëÛ¨)L?£ßuBžX?w.7µÕÇ?sDÆ50qã?£k{Lr6Ž?¢ççÊý?í¬2'*gæ?­ësî´È?'aŸ1}f?˜ÏGœ
÷–?¬ŒW.²g?¦õª&.½Ù?í*•wBy?¤¦Ø+²ù?ƒ¹t }iÞ?'þ/|	²Ò?´4%ÃÖP|?£^ˆD?r?êŒê½+M?¨Ýî;À&?'ˆžüXK^?ŽÅQaà?ظuIO¢?¨,y@ïņAGN4FGL J1030.7+6118¿ïù¨.v¤¼@HBã¼ÓZ†À:pöa7À;ÐÑPÀô@>/»"zù@™……žÙ?Âc'¦b*¿¦¿$ÝHß²?çgºú<q @ÐË}í@¶?ïðL2Þ¿èò‰?.i¿éüp>–©¿×ÿÞ<`Ù_¿ïÿþªJl¿ß&|¡;N‹UNASNone?î¼Äµàé?¹*ñeöc{?ŸÖɸv? Ã'¹? ?¹ÖàRå?·†™F¬o‡?ïL[b†T?''§lRÿû?užØk9%?|À.@Š?'èS‡?Š7Žëxi?í,r\=îx?¡ëÒôʐß?"4.î›wÂ?)ž$'Ü?±aaÇP?Ÿ·ˆ?íË~ºßÔ*?Ž‡Î¥2Ç?…2v''- ?n´Â:?­ûvÈþò?Œjì'<?íûÄå€V?º¥è÷?–ÁÓ#Ÿ7?¢>°¤T?±w­åT	?·EGÕÿò?îJ$rë/?ª"±ÀåÉ?ƒ†9½«e?Ž`ABÇN(?¦–í…²?§9BöÁ^?êòΊ?«Š=ÖÜ7|?§ªzæ›Âù?œAð'QÃ?Á˜æ°š?§
H° ƒS?è¶H³Åa@?ªC-¥u]	?¥U"ñ?"tGøѳ?Çà‡Ì‰þ=?¨Ç.<ÔF¿AGN4FGL J1032.0+5725?žòuÄ@I"~bÜn+À;<Uw*ÙÈÀ<†±	¢@@(²-9I"@ü¦y{ìà?ÐPP~?ª÷J=ªŸ??ÜÞÔa@·«?쥗•C¯¾¿åŸRu¿é|CG}m¿ã à_Ñ¡É¿å18‡0
Š¿ïù
By!T¿ÔcÃHê€UNASNone?ï¡dHÿÎ,?‰ù(ñþ½?b¿¼pÔ?fÎ1"‹1‰?'öþ±™¾?‡×?†?î]>
ú?¨#ý¯D…ÿ?' Âjí6?™ÎXN[ê? ÜÀá¦?¢Q¬Ó¯«Y?îˆ*ÆIO?–=è"=…Õ?…-BîÌ?…"n\`u?¢2/Ó\?"Ëà}T?ìÙ!,ÂÎ?"(¬PéB?¡
[á'Ю?…Ü'ïÄYÈ?°°Ñ¬è7?Œ9†‡¹µR?îӓüÝÇØ?Ÿ27u@?t»²"Ó–q?y½Té¢*? /Iܧg6?Ŝ\
¦?ëÐ#?¾ü|_C?«…Y¥¨¹?²ÂXÝ?Ji?¹aD®#Í?´a5›Šø?ík@]Nv?Ÿt<ì.6Ö?'åa,æt?‹ÜŽf[õ?°.•³"½M?šá)ÿl'?ç‹É¨2Â(?­–-Üæ?³''5ˆ^?¡ìî™9ó"?È'—-ñ?¨#0ü_'&AGN4FGL J1036.3-5833e¿ïcˆ'Ø'¿Ç;»cÀ5õÆâ¨eÀ9~ƒujæ(@ ï'v"ò?þAZ=c8?"+¹äŠ%*?¢˜ÕÏTçc@ü†~3â†@H¦³2œà¿é\P˜žÇ×?ڮפJD¿Ü
Æ(Ä¿Úª¨ À€¿ãʍÜÕ¿Ø\$"ô÷ŽUNASNone2FGL J1036.4-5828c?ÃkŽ	~À?Å7͇îÝ?R8z"A­I?TÿÏ^o'?ë@¾?Å9óh/¿?Ø;±_;­^?ÔÃû`g?žÁR"N5€?°ÓÙßÂ?âì»Ív?Ô@%ÞП.?Õ¸RòQ}?´5«øÒö? ®×‡Oì?™‡?má×a?ä^Ó?´†óè?¸?ҟ8~ezr?µ1­ô…Óˆ?—ç×kìu$?ƒÕÁq¸C?åñ%ÀU½?µþ½YV!d?É¡ZT›?Àr<rcR?NÃfh¶Ø?L__U"—?鱦¿ƒi?Àv¢ÚÇ›?ØbÐ¥'?ÒOèôr?¢öÚQ¦?¶n}"EëÉ?⟇òÓÆ?ÒÄ:˜"pq?Ú_'™"¯?¶@Ùäã?š‡ëgÔ¨?–;Ìèb?áü1[푓?µëœ!²wú?ÇxÁ:{µ?³É$¢éÒ×?Ÿ˜òˆPÐ?'•ýý—&?é%JéÌüŒ?µuÔ8¬ñOTHER4FGL J1036.5-1809?ë6*üOhÀ@AÃ\á'À:Ž%ߍ™±À<^E¾P2G@^û+9À@P1ônÒ?ÂäºiÈƃ?¬Bþ'Q?æMΊ<."@<>5šÁ¿Ó¢<UpË¿å««Ÿ«y¿êJ0'|G¿æÝ´"9¼¿î~"_¦XÅ¿ïìt½—$ÊUNASNone?ï¬Ôj·:?v÷U¶',?g(äØ3Á¤?a_tñúÇÈ?~XGzJ?r'ãÖ\‰?A',{Å?z/ŒÖ)Ò=?Yã
Þgbe?b,є´ë?{6{g)"ß?s‹'oì[7?ïgC§äNã?z˜¹¤˜Ò}?p` îÚ?kñ¢Ji:?ÿ
ñý\,?t~ï+iã»?ïÊWžï¼?f,ÿT˜åh?uÁ'Äì`í?Yüwß.?,Ö-æƈ?^U¹(S$?ï]è{e7?ˆ:œ¡sG?wŠ2§QÓ?s½6ô2=Q?Œõì•dâ ?ƒ0I­ø¾?ï4Ë;}.ª?""3d`›¯?p9ÿ"ÆI?y‰×ê,ù?•X£m‹|?¥÷Ã<ø{?îȺÜé¬?Œ_sök%?~6íÛm×ý?u GÙ<¥?ŸZé	ã;v?‡Ê;ÖxzÄ?î¾=ÀwK?…!æE'?' [iX?y°a›?˜p®tå3?|
Wµ/4"AGN4FGL J1036.6-4349¿ä
HÙÙó@):ïÔ8ÑÙÀ:Q-ÛÛ]‰À<Ab8Ú<!@­'¦Û÷b@CptÙÇ?À2­Ò5ÂZ?˗ä£-A,@	,辚Úâ?ý=e?tà¿Àõ5v¯_¿Þi%}½ðç¿ÛK-zâtT¿ã?Âùt7¿è¥¶ÞMþ'¿ðUNASNone3FGL J1036.4-4348?쐉_º¥®?°ÎëÔ?§ÝH*r6­?¡ÎãB#ä?¯!Ø+ y?¤Ž¢@mi¡?ëao,©?º­/šï§?¨ðT"Áhw?£¡Á3Ñ?¸|]§›§ö?¶Þvc Æ?ìE‰×¯©Ñ?¦z
ÈL?¯îr×ìn0?¢®µÆ²?«¸ï­ô»?–a3ÎCx?ê³|dˆy?'HŽp7ùÖ?¨*þ¦ ¬?€Ú%ø¥>?¾N‡dã¯?Žl4)Ôïï?ç'X5)?ÁîU"ZeQ?ÁúŒgq?¹ýC³Y?ÂáÀÃì?´³ÌÔ7?åÄF«àîî?Ƹꈰ¤^?½pÖ¢äq?¹y>õe­?Ê6ßgP"Ž?Ãahêi¾?èÐMBÜ| ?³†¡ª–3a?¿âîᵒ?°…J-'ã²?¹š§Ý:io?¡ÖMÄ¢êx?ä¬;ۀøA?¤Š¿%½?·ØuÍ/Ë?—́{Õ3?б€ëø·?¢Ì¨}¡¼4AGN4FGL J1037.8-5810c¿ïK4\\?Ï7äGè¡êÀ8¹Š>²Ã6À:_SUªL@±Ìp±m÷@z…\ '?ÁBL€·'?Òã%Ô¥ß@=B€®?ùÝ(¼Ü¿äÇÍ¿;Ò¿Û*«º®g1¿çƒhÀ2à}¿èeÌþJô¿ï›^?ÑQ¿ï¼~Æ.£UNASNone3FGL J1039.1-58094?¡ºã¥$?¡£A>1ë•?¢™¿ø?¡B"*Ë{V?íÃ(3Oã˜?«EîÉÖE?§&î!k}?©]$xÏ,?ÄCP¯rf?´eÅQýO?é|¼òOÏ?·g·Ôî~?¿"ÞÕ¤5?§Öv*?ÄN|ò'Nê?©±:ÚxZO?æûÄè¸÷¿?°"‰ì?<?ž¬8é¼­×?€Ý/š\—?´e«^Æ?¡1zК{†?ê]"Íړà?¢í'¨!>?Žyi*ó?†·rÐ\?¨£KÀ9?¦ŽÎ¼öqà?î—çòq?©¸ÆwÌ~ï?"ØÓ׈0ž?—*7â?ÅÜ}{Î$?»­Ÿþk£?éê4¸™?»Ü2t¶$.?´Â$'+?žÊi K4?Å¡;y}Å?®h\‰
\?è Ó.],ù?±á,‡È?~˜m毢?gRg¢™Ò?Ǔí§Ò†?­ÂÖÝ?éÞ
è™åw?®5HõîCOTHER4FGL J1039.2+3258?žƒ51Ã¥@Nvߤ?åÉÀ:¯û–ä³sÀ<©J–ý'@ҏ7@.@ŽIW?ÀT;ª·#?³Ryt‹K?ð4äù}@³¨Ž?ïÃùߪu	¿ÏZ|ù$ïy¿èL%r€P¿åOàèãƒÈ¿ç|ô¢©¸¡¿ïÿ€H»ÊUNASNone?ïҝÔ^3?p¹S?[¨¦áƒx¨?Rü<0oÏë?p
‡q]Ä6?j–œ±þø?ï˜ÀÛýÂ8?:æö6°?dRw
¡?gÃ''*6x?"»+-¸òf?z|BMzƒ?ïD¶Š/?'3=•DôÉ?v}î{è?t‡^Q¦?'Ýí•öö?{ö[@F©?ï+"Â7?tRub ò?Žð"RÀ`;?pÚ8Wζ?†*í+¡uY?bÓéßÊ°ß?ƒaƒ?{WÑ2öï?p°|‹Ì|?eĽëk?€Áàà(ù?tݵä3\?îÖàÿ"?švF®::Ž?yªó/ÎT?€$WuwC`?žÃ'@­åÄ?•ÐcBÍX?žô™½?Žî¹2p}‡?…·'_o›&?€,,ª•,? ˆŒ=&d?‡Iupí,?혖iþ?'ŸÿCªjE?¦°¾4u?ŽQ#(ž†?Ÿ›!©Ôí[?'ãqCÚAGN4FGL J1043.0+5316?ç!< ÿ@K[è>BZîÀ:ØâäfF†À<¶˜x1j@Ā=¨;@ˆœT?ÃO ;Ê0?Žü>:´m?Äàw9@@œ¶"‹ë¿¶ôŒÚC'â¿ãÝDÿŽk¿í2¬'ª¿ÚiVpOu¿íO|	eÚO?ÓH>Þ:KUNASNone?ï±øc.?ˆ?«ŸR?}<˜"`*?†TÊéÿ|?cŽÂQ{ú?eç Þ}?ïÁo­H3\?ˆ·àv<·?Sv¥Ö˜Bw?b¯³:ð5ñ?zj€ìmZ?†ón)ÜÐÙ?îòµ¼åÎü?'eÆ 'D0?só"xÖË?wÞÅÊYgì?œ¬cŠcÒ«?'Wn$@")?ïë/‰ŽY?J'_€Gž?U"Ði‰æY?B†GÙ³àB?TÕ	'?;IÉÓkH?ïr
8Cj?–«JU•‡?ŽNªÕMœ7?–ñøé%í?d¸Ç }?fñS×Òì?ï(Æäì¡?¦ûgÁ"Î?j
ÿ{W…"?ÕŠ[1V?—¥~5WS8?¥Ìÿ@ *Ä?î5*ï—Òð?™/ «*?€À2"zè?€`å?)̅?¨}DÍ?—ÔbX¿Ó£?ï±iŸUñ#?qò·—W\J?v›sƒµv?l‹'ùÄy?p°/ჸé?_çɃ'LsAGN4FGL J1044.5-1439?Ô˜ýù{¾@C©~+VÀ:ãwúã`À<uMËdíÀ@qÃ/?¨@CQÞïå?ϵ»£¯?¿3çmår?ðŽ†@ €?ú¶Qô¿äß,D+©¿æg öo³¿Öe:´e¿é
¸UFƒr¿åà#¡oÑÊ¿ïäê›íUNASNone?ïÐFÖ$?€†{±³‹?OXύJ«?Deoh_\w?šò¨Ó?€	>‰ÿÐâ?ï^	¿,·T?‹ÜFcýÜ?q'ê뙵?pÑ·ø¿@á?µºäà?‡H®ùí?ï"P•wS§?†dìS-?wÅÐډã?v‡6ŒL]µ?•ÄyRb‰ž?';C£Dõr?îh6î‡:O?ÅÓ4?"ú¹
5S?i/u¦?¤=âÕöâ¸?}{^fÛàË?ñk?—"1ßq€?duK[Fo?^)r9¸Cb?¥ž|;쓇?—·WHð?î8£Åú?¢ARß	¶?…ÈÅÁ`u?‰á9©4W?§»»÷JK?ž¨ÔžH?îJG¨FkÛ?"p''BÇ¡?…X疵`5?€R,?¦K–ÇÑ<?€,ÂÞ?ëôëÒ?œ(îC''?"^Äê?'Æì8Ññb?»Z\dQZ³?™'s–LAGN4FGL J1046.7-6010?༩Ž%¿z¿îócښë©À8"k·ÞþþÀ:lµ…ˆj@9Œ‹"Y@ÕC/Ш?½Ï€±@TY?Øm©PÆÂ@ܚ )֓@MNB«Ì¿ã:©´™Ð ¿Äo-ŸËaé¿âÍQ¢4è¿ê_Á†"¿íA(¿<¿ïÿÿÊPËUNASNone3FGL J1047.3-6005?£ÞôSºÂR?ªîmd&Â?冊û"?Éþ#(pƒî?Òw~}"Y?ÉôL1u³?·÷7L¥þŠ?¸yƒˆ6úü?ÖçÄw
Dõ?ÄzL?|J\?á6Úæ´?Åþ©ø¦3J?¹š÷õfì@?««²¸ù?ãÍÜRŒûã?¶Ðb)Q]?Ñý‰]ŒM+?³šŠ0J> ?¦s‡¬Ê2p?…Iø£h›?Ìä:âvz?¢ˆ‹@š·Â?ç_Âö_B[?£(à'(E"?¡E¹™Oƒ?»m¾ýßÇÚ?è5$¦
×j?ÆX	ÒøÇ
?ÊÙÿaà×?ÃY›è(ræ?šÏA? ´aO,?ÜSÿÊ-¾³?ÊÖ`pt?ác"yõ?ÊÅM>»ì?§/c÷Ÿ~ù?ž¬	Ðç£?ç8àïnQ?·å.ÿƒ¬?ÍP£F¸ú?µ«R©¤.?…›ªæª
Ù?l)eÅÒÀ«?ÑÚDL¾¨$?¯mó·=©?æ¼o.Xzb?¯'ܤÑÉMIXED4FGL J1047.2+6740?ä46+Ç?U@F­…ƒb°À;xTFŸÀ=å‡ó@ y¨ä^˜?ü'Dc_–?ÉXOwa‹`?¸.çI$â
?ðêÜ0@	LG²òA¿í$¼B;
ó¿áÁƒ(yF¿Þ€žÐe3¿â@¬ÞDïH?˜·G.%5¿êq=Å]lÃUNASNone?ïë¤ëK+ç?#‡¬Œ?0ï
$dé?jJFö°S?b=3E1wn?™Ú%_fì?ïâóª‡(?lزұXt?8Rü'9?D]jž
Ž
?jñ¬º7¼?iÏK,þ(£?ïdZJ¥7?ˆ²ÿP ¸?]
÷äLv?p"cg»s‡?'£à\†³?‡bqùï$?ïí0pFu?F砊ØY¹?!»ÜT?m¯?‹8s á?aU»z{-?F²‡äð.f?ïÜ×QØ\?~QâXIÍ?:$ÛNW°À?P,ýqÔ?pZƝ¥A>?z…j4•?qÇÝ>?‡ÊçµÕf?K+L%Ve?Wâ­Y ø?‡"®ØOtÎ?…È9[ö‰?î¸ü\¡/?•˜ò¥'?a³Ï»y?pYYp¦?£Ue
Ú?",WòD?ïÁôK콃?h¾õÊK+
?6è9'"?1ÅéÝC?}—Qú?h]­™AGN4FGL J1048.4-5030?àe¢ïX½Ü@èϦ›áÀ;~‡Å[¿À<€"Œê^®@"ží'`A3?÷&Lëk…?Ùޘ§+R"?Ò¹Ù« ê@•‰ïØj@@7Ӏñ¿Ó@LyË¿ài}Èâ¿ä§ü~Y®¿äHxÌE¿èè\૦â¿éMŠ'$‡õUNASNone?ì(æqu?³Çîýµ^,?|0À"mw"?põŸGË÷?¼üs ¼–§?³YñYÿ7Ê?à‰`ÑÑïK?Ì&ÜôÉQS?¡–<U?¥+­Ç'¿ú?ÜÍ›"?Ê튬Äû?ì 5Œv<ë?¢MÞb?‹ãȨ*?"ø'Å·Q2?·Ú‡¶ÈH? Æ¨yn?約¶!~o?´ÒJc?Ÿåÿ×CÑÅ?'p
vÀ¸?Í1--¤lË?´ä:»¿ ?ä»ÅZ¹?èÏíh£­?#õT_»˜?'mO…Đ–?ՏVLñRò?Â×B¢E?Е°'÷?Åsä¡P?¬àET¼Ó'?µqMLÉc4?åçmRqo?Å3ÿì‰Öƒ?頁?Z´?¬€ëèdæ†?—Ľ¹ÓY?"èùƒX?ÈÖ%cðH?«=d9o?Þêç6}?À¢öm7Äp?¦m<¬IC?©´ú:qª?ß;†m0É»?˜ûäèL…MIXED4FGL J1048.5-5923?ØÚç¡S;*¿ÅU€e-À8µýawÀ:Œd×-©@Ì22Yò@9fâ?¿äð/'ŠÞ?à€`b–M4@èîkƒÙ?øœ¤Z诿ݫ^ʐ²¿áa%Ie¤ ¿×ÐfíÖÞ¿êS恩¸Ì¿ïÿÞý¦ßR?ïùT_}¾óUNASNone?áMÀÛ°s?—Ù£þrâ?îtúÔO«—?¯ÿYUË}[? ?«ÜO<L?¨±€Ö()?ªIù»pÇ?²€;ÙÝÇë?Û¨MdW?ÇÉrOé?à‡^=D{|?Ç<Âå(Ÿm?®e²[cQT? €oŠ©*?å½ÉnÉ?µqŠ!è™B?ÒÎ"ã.ä?³|W­½B?‹†ÅQdi?rÁv»ÝQ?×®ÿ³â?±×f(Fþ¿?äêelží?±ÀÝ$Ò«?~áâ#ô@w?ƒ-|45ì?îà5Ð
^?¢®,+?œD@»uÑ,?Ÿ?ŠŠT?`!¬6Ð?˜Rw?S\[?ß2eœ«¶–?Îø…¤Ö?ßâ™V—€)?βuÝ
? )2ç#‰I?"'~Îet?è1±O1°@?´OZbûa†?Ë.°?²¯ÿcWP9?`¤;ÀiÌÖ?NE"»#š?ÛV"\²n¹?»mÍôü'?âDJ–7už?»bÌ(8žMIXED4FGL J1049.8+2741¿ì݈À>°%@O‰\Rç-¡À;$jÈ˶LÀ<ÂÉø6{@Èey+ü@c'†Wv?Á?wd:'"¿ª†»›w_?ê_
Awn¡@Qu=™¿?ï¤nß±¬¿é£=òÔÉ¿át€Û\²ˆ¿ÞCO
)N®¿èê¢5Ié?i…ÖüíUNASNone?ï°9ëÓ<?'vDáΕ?bÆë½ ?U]s6¥ ë?~ý-–$ë?ºWICê?ïNYM?'ÀúçÑ?\X7¼ìBQ?a‡Jvyb?…4år²f?€1Ü^η?ïcT÷™Õ?€ç¾wjáÈ?d—Þ¦†{?_3•d©?''4yä…?XšâÎ"¯?‹‡»©?hÇÚÇ!Â<?lÖq8>òA?P›J܍®+?ˆ ֈ›?g\XÝpÜ?ï%
Ñj@?"[è%…?{þÅ'?p͙´p,\?–;­bö°¦?'*r©Çh?ïgR8?–U·œ­Øè?g5UÚJŒ]?rîWŠK5?š"î±pr?"*µlP8¼?î•ê.vNÖ?"cTåµ|?t­n$ƒ<•?qYæ,BžÎ?¤¯W8N?'ꀨ63{?îAc' 	?ŠWÄÂO5ì?‡|ؼÆϛ?r) é7DC?¦
—ÛïΆ?ˆóÉqë®#AGN4FGL J1049.9-3658?àùØþ@3ÒóÂÚۃÀ;o…j7¬?À<½¯€‹¬@ü<'UÓ?þ#Ÿý`éO?×îS/Qý?Õ<캨ÝÚ?þs™õßëŽ@nÏ[rl"¿Îˆ""ꐭ¿ì6J	8æ?áO܁u¶f¿âÉ­"K¡¿¿Úû¯cZm_¿ïý_ ÷ÇLUNASNone?ï€vÙî¥?±[cšh¨?]¹Í@²?PÒó0§{N?Œ@²«A{?±`Õ#¾b?ïysüƒZ?‰oä¯æŽÊ?jz.ÝG &?p͋Ýòû'?‹°zŽ?"@Ç7
ÿö?ï …­9Æ?ŠÎÍ+$C?uHy¶cJ›?uƁÀõ'.?–ùÐ×l«?‡¸?Àííð?ïñ`]–g?w@¼jøÖ?be	§Æ?M½`m~*ò?œ'Q`lh?v>I`¡ù`?ï8p6],?£r'ƒœdø?no‰]0ç?c!3V¬?•$Öç?£W¸·T?î²æ2é%7? '&²Â¬?zâ"rÛ!?ƒÄ=ž>˜?¡uX'ß),?œ=.ªOƒÓ?î6}hò˜õ?˜¼(Vª>?f֍¡y?|:¨Ä™m?¨«N³þZö?–Ôçp‹/?íkŽ÷T4á?•îÙúÎ6?l/20H"?cü,Ü62?³Â²ê0\?•sÀ°ÎƒJAGN4FGL J1054.0-5938?ìøFŸezG¿´ê}6âjÀ:*&¨«À;zKìgœÇ@¥ðj
à¯@DÍ$
¡D?Ò=Äòø6?ÛFuš¶Ð@	Ž"ü¡¦®?ÿ[Fo¦/¿â¿°"—ª¿ààŠï²ªã¿ã ¢Bµ‡¿àýT‰Å@¿ì¯¹"<¿ðUNASNone?¿Ì1¯q?³í¤Ãœ·?™SÂs"N™?"úôéW?ë;áÆ6¹-?µ¯µk°rç?ÐV0ãŸÏ?Ã)U"ù¼?¥# Ê¡? Í¦†Nÿ'?æƒÅ\kî?Ã#ò:<f?Öª­ºÛ**?±szˆø±?¿5+pq,=?£¨·áܓ?àijúÕ?²á'hGê?ÛX98A?§Tj"Ü;6?³Ò¡ë%<?'"-¬§?àßÏ:ˆ?¨lõ'z?±¿	eþcR?¥¡zû?£©FÌøSª? "Ê®¬ª?썊f9´›?­hAûփ8?¹Œ;ו!?´Û&9¢#†?©ŒJy†7?ªOë/üV"?ë5³ö½9?¸8κT?ÇÍ"
4á?«–æ³i)?ÃóEãË'A?ª6¡¢Ãæ?åí¾‰è÷?±¸ºU?¼G?ÇáOèÂîõ?¤—³5XÉ?·\Ýï$‰¤?¡jÉ!b?çHfdþ?ªØj ñl]OTHER4FGL J1054.7-6008c?ï«D«-–¿ßt_ƒVRÀ9>¡ò-¯fÀ:ºôƒÊû;@ ¬ÿ"Ë(³@#éÁЈ?Åß¼™Ï?´}áWHfK?ôc@\¢@x•±'™¿é–:‰hÊ?î6êx´G¿ëB‹`òË¿á…!ýÖ¯û¿äw'¯c¿éÎf*…UNASNone3FGL J1054.7-60064?ǸÔîëkÚ?ÀHe5À+?¿ŠÀsB?|Ñí]W?éÒK®Ì~?ÀtÑ|S?дlkVK?Ǭ fÊ0Þ?"TŨ`ôÇ?˜aeUT¸?ç#'ùŽÄ?Ç. Ö˜?Òf"´õ?³ä×{­?±@BK2y?¡1>t+ŒP?䤭Ü30?³Æ7$úù??ۇIó
›‡?¨Ì΃2? »Ð:ÀpH?'²:¿_w?á0žch?¨æ«6£Jà?ºñ·ñQ+?´pÜÛŽK?†õBî¯N ?‡f†¬2÷š?ìEóöm–B?µŠø"-Tá?Ã"~û?½—«WÝ´?Ÿ‰ÿš?áá?ª+ã¢k?ê;}·Ìò?¿*A¥šas?ÄÿÍ//»?¨õÎy¥Qk?±¾'etw?¢â+i÷PÀ?èˆIJÕCò?¯ÞúÚxÈC?Ë2dÅy?¨ôâXŽÝ4?¨/]:àS?"[¤èÿŸ?ç°q?ªÛ×]µ OTHER4FGL J1055.6-0719¿Ú'IÚI?@FË  ôØÀ:Òs«ÉGÀ<}4#;z@öõtŒ?úfÉèì¾?呈pSO?ãè›)¼'ì?ýR0",J@"B)›.ð?ï¸;Ÿé?¿á jÓ¿Þ*¤ ¿í·¬ª–¿ïêԟ©þí¿ïýÁÆßMUNASNone?í•kõF"?°Ò.VA»?}b	ü÷"?zÄsœ`nj?±~ÆÎtÜ?®ÝöÊ/
E?îJ[¢ä`?®,/9ÒªI?",óº2§ƒ?I°ÛÒ?¡CËÿé8?¥"¶Ev×£?ìT/äcM?¤¿ur:3? } U»8?"ÒO0‡?µð±€?¡Ck­«§í?í
¸ô¹áõ?œj'Ëcû"?'¹@7"yí?ˆ¶*%ÔÏ?²ûèL½Å^?™Ñt¨k*?êk˜3µ[Ž?½voTîç ?'ki<?Žd'{È5T?Ä=ø"Ÿ?¼½ß«™?발Ä,¦b?À9·K?§{ÆMÛ?²¬XûÿR?¶½6Ñ<7?´HŠß‰ÁI?êgño³0?ªa-"™ä?¥ýñ7ss?—Û¨~?ÀàÉT®iF?¦ï	\¦ó??ë/Ԙëk?°a""¢?Š«—çË}X?"¤sô5ÊÒ?Á—G.è ¾?¯z€hVgAGN4FGL J1055.7+1033?ïߘýp^@M¶0©8À;mv"Û·À<·þ^?Px@L)ÿ'׋@Õ`EK?Îú0³&2š?Šæ
²ûj?¸åõåZ¸@xއ_ZY?ë;>À<{¿ê©p§2'?²zò9˜Ó¿áöRš™Ê¿àsø^K¿ï—m¿öûuUNASNone?ï'.c?À_?¸®[߯"?U$xÐÚ
?'õvÈáì&?ŒÏØ,íÂè?¶ª–íYï'?ïƸçùµ?‰.ČØE?E(‹j•X.?P\ÏrUÛÚ?yþzƒy¨«?ˆX*3fQ?îæÕkE¸
?•ÜߛYØÑ?]f$Vá`?fÐÆ´^[Ë? §x&ó­ä?•·æËKym?ïÃ8ÿ¥è?]iÌe1|·?H®¼ñ
Ô?3][¯×ˆ?{M¾"t–B?\zrp`"?͑©ò?žý­¹bìò?L9åAŽ?iz¢í-%	?ŒŒîMk'Ë?œ\ºáªäÌ?ïA³Ö©ý?§éBÄã®Â?U|ËEÞ¢?bU Rå?–q¸ûf?§·ìÏC?ííXQ6Á? -¤Ó?doÿ9Úó?i®u TÅ?¯ãzù›añ?ŸéÖ#áÒ0?ïQåPÐä?|0k×í"?YmÊ°SI?Ncý<Ÿ?",€îPJÞ?{ikù(BAGN4FGL J1055.7-1807¿äs*D!B@Bb¢"ÕÀ;†PÎN­À<¦üZYê@`àëgÃ@T"\Böö?Å
{"Üß¿·Y ¾Í–Ý?óUE¬²{@'óÒö­?ï'S‰êÏí¿ìîbHŸ¿áé€C‡>¿ã")Zl] ¿ÏfD˜
xT¿Í^;I­UNASNone?ïCfŒ{ùÌ?"»k'"®?Z	sÛl?Pg"!]µÍ?•òœ'±óÌ?"Uç@«Æ?ïK–7ԏ?"h‡‰éѪ?u~|7r?}~!öwN—?'-™ýRâ·?Wªi˜?îôá09È?ŽÅüèÂx?j
B.'Îu?pº/PLŒ?ž"–Ü9¢?M‹/:ل?ïM|+÷?xf*¢-^?WìÙõæ´È?F²(ªÿd?"Ñ­6~?wëv‹ðŠ&?îø$-K?¦	œ}—?qz†Ýíïý?hz'4Kê@?¬‡Ÿž¥ÎÚ?¥ŸúFW¨3?î'Rr5?¥´Dð¾Ò5?~EÊnáz¨?
3Ê,Àp?¤‹bSš?¡æh	–¼!?îY³5Þ?˜+	3©|p?p@Âœ#?oSS´ƒ6?­R²ØÄx?—q×ÃçD?ìñ'fæ?âÆ֋ÿ?x	NÅÏDY?q´\î4}?¶öî‹óň?4ž˜1ÁAGN4FGL J1057.6-4051¿×÷ZP@1«\9¼ºÀ;T'ÏR¹
À<¯ík¨Å‡@!Å.	¹?÷ÏY­€?ÕÛt/|ÅM?×­ãænß@®¤Ã™Gd@ЈÐº%¿ïÿóÀ¬ƒ?ïÿÿ&¦³?Üe·>ñŠ?œÖƒb~-
¿Þqá">éu¿ãJ½Y<\UNASNone3FGL J1057.6-4051?ïӁ?x÷õw£n?K[â¢ì/?X¬ëÔ¤…z?sú,þ"?v>á	RÚ?ïÇ5šä?€Š³,|²œ?P\Áî,j?[Š‡¬Öèþ?x_4ÚÜf¿?|Š¹W©"?îWÆv­—?ŸføyÒ= ?…Òßï	?Œ©$ÌÊÝ?¥àœÒ"?š™¼ßuÏ?ï#£N+å•?w}Ð,T$ ?cÑÏ Õ.»?Jô[ôˆ\?™\]sڊ?v¬ŒZ'Ô?ïÁ 
™Xy?{O·â}¸»?XÖ·|A·?\ÂîI¿ý?xúLñ e?xìƒèז<?ïe‡Á?'õà‹SW?dr‹˜]?u{*™_д?ÀÊÔݹð?Žô¼ÿ
?í÷ñ¾F[? NyâN|*?ƒ´Þ–fDì?‰›ñ¶Ü¸?«"¬|—¢–?{ºðÞ"U?îD~è›é?'I¤ Í?mZÙ%å†?b¦‹í=?­6
'Sƕ?'¿%á×AGN4FGL J1058.4-6625¿ïQØMŖßÀú†×6&À:©ˆúååÀ<@—ŸÄV@ –|¨È?þÄâ½ÏÙÈ?Â%;8eL5?µ¦?piu?öóFc'ŸÐ@à¦ÉWø:¿ä|Wisa?ïò±}»í¿æŒ"ÎX¾¿Ò¤e¥vF®¿æ,SzÑWv¿ÙÞ¾‰¾UNASNone2FGL J1058.7-6621?îÖÙV%¯?¡hã«KøÆ?h隩µ(À? "ËCü?¡ÐõÕ?*ï¬p—à?êQ]‹G?»²±oÕ?jCÕM=
N?sh¢:Xêž?ÆQz}ìâ8?»=[Ú`"?î4%	Ù?"ù"êª6?y¿9Qçž?qÇä6÷"?ªäÝt­p?'"œùw/?íz;…ð¢ó?‡¦O~{,²?',<kb›ù?o¬£È­¿}?¯Æ)føÿÓ?…‰è°ûW?í5Iý"Ù?§vRdù?L?~M"¢¶0¦?–›-üDA?µQƒ‡ŸÌ-?¤"32µÉv?⃸¿_–?Æz‡\͂Í?ušÉp}Ó?XC"³â?Ú¢#¾Ÿ¦?ÆYزøÕ?ëNc²¤O?¥*õˆ>
¾?‹! ‰È²?}w‹L°Ïð?Â¬oÎÞº?£÷eÎL9ü?ê	ªWú4[?Ÿ{¥n¸:1?£§†ºka¨?‰RR³+;?Âïtñ³Oè?Qg8¹ÓøAGN4FGL J1058.9-6101?èZh'º¿ñ"ӟNå@À9¢G«<#À;$•%–'~@…¿9fS@÷xmži?Êðmü1ê3?ԘL½rç©@™È î!±?÷ê–߀Å¿ïÿ¸8º1?ïøVˆ¢ÑQ¿à2Û>Õ}Ë¿ã<æp–¿ï—_'œ}?жƒ_E‹UNASNone3FGL J1058.5-6106c?ÀÜPòІZ?»ÅoÅY€?¦ÿ#Ù?¡l(GFæn?êg[Ñ.}¹?¾rF¢~?Æ«^ÙæL?¼òËJQîñ?Á
®vAó?³"vÀÓ?漫õð:?½ÅƬ­?ÑPy¹™-'?¯g=Dç¸!?ª—-X¨¹?¨¥˜
Â4?â­WÝ?>?±«EoâR?Ìs a67?¡4Ñ^{E?ʌ鲻?¢Ó·cä=ó?â1Ó?`EÄ?¦K³˜?®ðN)}?³!Ò¢¤°?­¬òsÇÅH?§¾š†³Ëº?ì6/¨ueÄ?·ÅSÝóÀ?«XìL¼=«?©a|e¹ê³?Ä
­˜p?»ògúÝy?éGû !?½'ÀŠÛKý?¿֍jâ!?£~«!nt.?Åo†¸7á»?®…ٝe?检ά?±Õp8Nƒ?´.e5÷¾?"ýÄ©w9?Ïúù'ÊêÂ?¯XUödr\?å{t÷½€?°ÝDǹOTHER4FGL J1059.4+2148?Í!ñ;ý…@P,{‰
ZÀ;N1‰åÇpÀ<•ÀY÷Ã@ddàÕBg@îà¹Ü?З¶€G7?¹d
ý´÷?èñ'?_‡?ìKV^~ª¿Òn¡¾/•¿ã­`öºÝ¿âл¿^OA¿éšº–icq¿Ê÷‡‹z¿ïñd "‰UNASNone?îþ÷•´mì?¹J\ÏÂS?'±•îý?¹4bFó}?Ž(·c–î¾?¦µÂâ@¼?î§VéÔÎ?¥Ï¾Ùö?ŠT¼îC?"ð£EÞ¿:?ë.ß&ñ¥?žÍ¼OÀÌR?îŬÙ§"?'K¯½»'?"vƎÏÑ?†^7ÌR²?{×Sô?ŒAd~x¹¢?í"³Â à?'ÝäléœÃ?
ªÆ7E?}(²gÏÿ©?²ç·7»ãX?'TP¨-?î•Ê‹ôÚ?«ž\PQÀ×?'į?pÊÃ?¨TÉÀYË?¡ò3ÕÃ0?œ'aõ'²²?ìR²‹>HK?¼ý
ØìÑá? åN#ԏr?«7×P˜Ñ?´÷Ēk§ï?¶K×'fä?íÄop¿÷?›Rµ´?'F¼é/"?·‡ì ?ª•ª‡ä¡'?"Kpúe¢¡?痚´Tc?¬•¦8$?¢ˆ^ýŸ$3?˜{59úuó?Ìÿ}pƒ=?«ça–¦}¶AGN4FGL J1059.4+0226?ë]R	HdY@JɏÙý7À9ÞkÑà2À;òhÒQq@‡séèw@½‡Ý¯s ?ÄåýJn
O?Á9ul"§?öÿ\‰ÉB@I¡yŒÞË?ïÎ` ©®¿ßè©¢%YV¿ßÙ=ˆ÷Šæ¿ãX{Â=ä¿ë²‰ŠWÝ7¿ÞAÜCbU`UNASNone3FGL J1059.3+0224?ìƋ'ùJ?Ʌë죫?³Ü=;Ìi8?Éð1´`¢á?—½˜¯íK¦?"…!¤.2?ï­IÊ×Ý«?}—]og?_"mu?d÷|)Åkò?€ÉL¯B¿?uób2±v?î4¼Áx"?œ?˜A5ò"?'ëNñ}ý?Ž˜»aæ0?£¾t>r)ß?•¾p;òâp?î…@kÕæý?}tQmº$?‹—¹Ú&³?i¿þœvmn? Æ
Ʉ.S?wdÐ×û×`?ì6[9è?Ä(xAD™?²*ƒÜŒì	?Ä|0C$þù?¨JB"TYi?¡³Ý¯ÌuŠ?ïaϨÊ9?—	M¶¶Ñ?rV¼O©?{)…H?™oðX<œ?"6#ë|O?ìøýY~îÀ?¤Þ¹o‰?˜ƒJ§âëD?':ÛH:¬N?²BˆX2?¡Ú׆ÌþÅ?ìCÅ6Låƒ?•Ý%Ì.? ®ܹ¸?ƒo>‡"Gq?µØBtQˆ?'ûÀŸ$ÅsAGN4FGL J1100.0-2044?ëù£æµ½M@A‡´€¥¬ÍÀ:ÁçIOÕ*À<"÷z€Ï@@¸žÂx`@SÕ4z[?ÆÆl ¾4?¼C"Ó†û1?ñu~æ­?÷µ×8XŒ¿Õé4 G3¿ãgšx
ÿ¿Ùsÿ*¿åÑG@~š¿ãæàtI~¿é¼«aÃ'UNASNone3FGL J1100.2-2044?ïpœMö?}=OÃl?M÷¢Ó'á?@Žÿ(EÌv?†ÄƒÝW¤ü?|,§+;Ê?ï`ÒO'/?‰D؆›8v?rpw–Jhß?rŠR–ˆ<¯?Ž"0r.]Æ?ƒ‹Â´L¦?ï<<÷'-?"EÇj_2?t—=‰!v"?u.vÅ`=?"R'§š©³?€</Ú?î'ßå>™Õ?}•Óß	>.?‹úíFr…?md)aW—?ŸÆŒ•ð&?vëùà¦ñ?ï,.²£‰e?Œl{#Bíi?`\È?Ì>?R5'—w—o?˜n›2à?‹¿ò)ðµ?î4ôå€Þô?¢6ÂÁ¨xÒ?ˆ•‡ì<?Œί8ó?¦¨ÌCcLÄ?¥p´À^?î‹g`ƒ×?'½ó¾v?'ˆŠ²»?I2%҅?¢§ƒªëÉ?ŽßV²×=?ìdZÀjé®?–âMÄWS?ž-ãåx™?†dEZð??µQ±ç"i?"WWAGN4FGL J1102.3+6715?íÙ/<Q @GJ²BÀ;è¤nòÀ=0fC*÷û@!PØ?ɵ?ûV³»ƒÏ-?ÏAÖçØÂ?¶î•ÊW&­?êö5çB™Ù@ÓLÙ!™Ù¿ï¥íÀ7h!¿Ô°oó ?ïù0¾
í)¿æ{›¢|K?¸Ï2ؚ`¿é8%@+i:UNASNone?ïåê½EÏ?]'Ã8Ö?0çÿc€Ò?'W0è§)?gø`héU?[Èt`"?ï×!͸¸¡?wðب̵?BiHñà©?RMN~Œ?r!øõµÿJ?u76†Ò}?îߔ#§¾º?"Ô'ôr _?sóÅ,@
?€Gqô»L?ŸŠDo¤0?'ü]îy™?ïåÉ¥rb@?QÉcÛw'"? ˜ Ñ\¥Õ?Ú¹ˆXú?i,Ød~Yu?Q}»YY	?ïÎ'—bv‡?mCTu›‹(?@Q)<)i8?8—;⤳ ?vâ.e%ñ?l-žÁ#?ï|/TÆÄ?'GµYQ1?SO°š!¶×?a¬ãª3'?ŽŠ4¾üê?'>uý_s?í㤁ÌjÊ?žƒgÕ±ŠÃ?zb™œƒŒÈ?ƒ1åýÝÕ?®yd²›Ê?CÉôý?ï´2RžÄ?rßHqÍ?-öˆ)Xíu?1ìépgV?'{'1EfI?r¯M/ꛘAGN4FGL J1105.1-2600?®éœ·kç@?â2ŸÀ:ŸÀgnÀ<'•=†Æ@'ñ§Lµ@(í½\ì?Пª?ÂpŽHÌ^?óå3E§©þ@ÛÃ_»§a¿àÕd¶býü¿æ6ü¡%Ôü¿Û"ɾO†{¿ã/ýÍpa¿ïÿoì÷å¿ë¡;NŠ§ŽUNASNone?ï{ö±€HÃ?Jî÷Ö!?l9eÚw ?c@*8Ìóä?‰óï•=ƒ2?}yH¾zA—?ï´ø¤Zׁ?d®ƒs+?^Ë@¬'Ç?h~+õ"?}ýû ¥Å€?v(P&Ä
?îé€Ú…òô?'å.Ih?†¨áݖxÇ?…à	{ºò–?—{s½É,?‰‰}@VÔ?ïNüþÔíê?neóƒÖá?vñz/¶Æå?X­½Ý''ê?d"EE?hòó0Èx?îv|Žh—?›8ó9éÍ?'ÍŒû"Ž?xMá,{Ä'?£äÔ§ö?˜#âûeÑ?ï,7Jfg?•fÂ|Ò'?pªfÚKXÎ?{I†WWµ¶?–N"(‹gç?'@Ž·ÿb?íÝ;›ü9;?œYsâñit?½'ì25
?‹ÅK©?¸?©Í}F³µÓ?—'
îîI?îbG­é‡Ä?‰¶w Ëg?"°Õ	,/¦?uŝˆŠ?¤¯OÛ¬Ûã?…œ‡«AGN4FGL J1105.3-0626¿ã¾7šdßl@Gß÷øʂÀ;¢HÕ[èÀ<´Ãð…8º@#P׿ïï'?³k=¯:@?çµ+ÆWh?ïÿKÚÉå'@""†âÞ?þ¾+õ&]¿ïúìšÈmÂ?ïØQ?¸§§¿ØŸ½J"ä¿êèD§¯Ý?æÑò¦{)l¿Í¶¥CÃUNASNone?în'+"÷?³Ý\Åq"?ˆúˆ!1<?¡šF¢å?¢ØK@|9:?±†6v,Ù²?î뿼̂-?©…灡-Ì?°õîfŸü?Ž誳NJ?š›ÊäNÐq?¥5±ŒuÌ?ìzé)Š?«5†lè¡ð?›ÏLãy?•®€u?µ;Ž¥¹|R?¨†Ò!ãd?éSCÀ°?µeÜçlÎD?VÀ.Y0Õ)?`sEñ£¯?ʆmb.u?µgR…W!?î(Éb_Ã?®zÉ®a=?—kHbS;?¡€UÁK¼?¡½Å§L\:?¦ß[-˜×Œ?í]ŒšŽ?»ŸOCy?""yfvÁ"?«
è\èfÆ?¯äú"Ú´†?´k-Š!¸?ë\'ºäò?°:øD¤é'? "4VuŒÝ?–ؤ¹‹¼?½
§üfv	?®áb8·à	?ãÁúŒVBµ?ÅÿÐã»Y?R7wO<µ/?s¬æûéš?ØiÓoöp?ÅŸÁô#AGN4FGL J1106.2+7303?ሁŠÈà@DüM:'£À;þ#qõÀ<5‹¶'@'Ÿ‹¡y@ãÏ¥Å!?Å^BÀïÉÒ¿»'¹5Á-?õÀ´á¼©@«'â[?×}_*ÝÏ¿ë3™àf\«¿í~ÞAê05¿—'n¯¿é[Ŏ*Y¿ïæöäÎKRUNASNone?ï¤êOêy?x‰«DNÕ?h¯ðËÞ©?gŠ¶V°'?€™«Jæ•
?‹/ÚüûÂ?ï¡7³©ï?Š%‹"¾[?gGMð™r½?{çìå{WU?à?‹Õ7Š?€+
³2?'ÐCò?•òVL§sX?w÷|%Þí?y¦öêќJ?¤#¶¤¨}?"3Ct*?ï–Çqª¬?s³¡œ	Bï?hŽ˜PæB?ZÜ6â7?"*¹C{h?p¾lèÛ©
?ï4œ̎Â?œNîeþÖm?'âzɠΑ?'6_—{z?ö€ÄCbí?˜´n ÷	?îÿW'ÒÄÍ?¢Yfî^ˆp?z^¤g‰?D?"ùn½éS?™}dˆ)Œ?˜ÃEҁžy?íl¸KÐ&ã?Ÿ"ý55Ç?ˆú–Mx?…CëDå•Ï?±zê×ϵ4?œøØýa¹?îQ†BNÚ?™Bh¼IJ`?'äZQ?"E©À?¢c)­
ïÌ?"ú…äþ>VAGN4FGL J1106.7+3623?·mTþ³D~@PŠ\å´$À:|ƃÝo²À<]˽Ù@ø³"כ]@îwÐÛ?Áq56î~£?¡Œ ?ƒ¬%?ÞwÒ>Nš@m«ÿøž?ïÿÎa¢\a¿àÏÜKÅÑ0¿æ÷ôގÁ#¿âÝ­Å ˆ¡¿èך@]".¿ïþ!nÑTUNASNone?ïîºÏ/ŽÊ?VØÓØ_Æ?<¶w¿_ìò?2P5{pߕ?[\Ä@À?TÌ꣨3?ïâIAj?oNvÀ?:ÃôÞÓô?F•¦ÔðN³?jŽSeÒ?kÕ|õý#S?ï}s`þP0?†lz£¾ú?[ý6͇?bý…ªïi?#€ùê±?…ÅÄá?!]?ïé
­	/v?F:qÛ4Wt?F·"¥ß£?+bT\¾Š?al$üƳ?D.©äašà?ïÛ¹æý?oqÄàEV?P;3¨áDÓ?JîDMþVþ?lÑO¢Üa¶?jðv–{B?ïžs§±N0?ˆZ½›ˆ?LäH"kfÑ?X@ÒÌIÓá?†"Ñ"ÏÞº?†ÎòœA•?ï,ÐPԞ?ŽÐ={¨ÆG?h
r4÷í±?jß׿
Á¡?—|¦Ûc£?ÿk¦.aï?︎Å]Ë@?f†\)'hÝ?aʲ¹Á?L'ÇM'4?zӘôN53?dîñ@ÉAGN4FGL J1106.7-1742?îv;NÆȸ@C=À~à±À:xø‹—xWÀ<†]Ötì@‰ú‡;?þë'*ç?Ãì[!Ý?Ùh$¬‡³@pÀ\|@Í¥u«¿æ¤;~[O²¿¥~ŸBP©¿Ö¼ð¡=Qð¿äó;Ì_¿ìƒlfZ§ì¿ðUNASNone3FGL J1106.6-1744?æ¤Ùù'–?Âå-6§?Êz|ªÂÙ%?… ®ÔÇÌ?µê_ÚC…?©$δŒØ?í!^#÷«ô?µzǔ¦+(?¨G¿ví'?¯Ê§w1ë?¥¢^I˜l¡? nÓü¤¨W?àÅã"íëß?·¨3"b?Ö÷?îhº?·"p]Ú(?½óãží¸Í?¤Vףђ?ìû‡¸pŸO?KŠÄžèÔ?©®l›{õY?…1€"Ñ=?¦™Ú
y¶?	#À{'?á!ò5×?ƉñÑ-"?Õ8ú¼ÿ ?Ǜ'bm³b?Á!'À¨ëá?³¸pÅ?çÒÖö‹%ý?ǀ'©Ÿ?Â*ƒ1±?ÂúNÿÜ2Š?½B=xl´?´Ÿ-‡k§?Ôç&;Z?ºI#NR/?à?	D??½IÞZW©?Ãð·dÓ
Ì?ª™ÂヷI?骚nù?£03'Œa?¸–')·ö?œ''O}‹?ºÒ	Þ·A?—ŒÑíŁMIXED4FGL J1109.1-4853¿îëãÚ@¹ë@%8ñ,'¦7À:eÒ(V`_À<,"d®ÖB@ˆ¿¬¨À@Ùýñ7?Ϥ4<ȈE?àãm"BJ@€˜@Ô¦@lLJ±T ¿Ê˜ÊÔпÀ'/Cå]¿âz•ÈSÁ¿â*þ~ð¿ïڋÒ0¹Ü?욉¹QÅÅUNASNone?èè$Ʌfÿ?ÌÀµe/¸2?£½g§tœ·?§P]U9¦?ÇpïhO—?Ë&bY*W†?ë/5¸§.‹?¾áAgÃ"?®²Ð Œ•	?­2感Z¥?·,éèÈs$?¶Rx˜¤|?é•
‡S­?­½ñœÓ6?³øÆ$ã?¡mž¹Ë?¿^å¤Æ.´?¦áôO"S?ë^Þó&9?š«£ä™?©WJ?§%?ˆ¾l"¥Yƒ?¸da,§?"5UÈž?â¸W¨ï‰!?Ŕœuõƒ?¼éV})]?³;Åxl»?ÓTû
Á£h?Äk†Ô΁‹?äÅÓå"Œ¥?ʝp"»ß?Ãn%t†?Á!™xªX?ÉÒBFeXä?ÄÄí@	Û?äh4',K?³ä_@? ﹶÅy?¨·A_ƺ?Ì>?©–Å\?°;:­e?ãDfètý?°(4l7C‹?À•ÌzÂhñ?£ 9'Uê?Ñ,ôôÍá?¬¤-)*‡AGN4FGL J1109.4-6115e¿Ø,"{Wí°¿èÑØ8såÀ7C9+À9ãKÁŸr@!ÿr:Uf?þÝí¡Xª¼?£&"S¼ì?¦¯
šÜ@@Sý®(?òIK :?îT­×>?׿à'°+¬V5¿ßc? (ÿԿۛ㪵¿ãÍ®oê¿ÚpMû‹| UNASNone3FGL J1111.9-6038?'Ve.™?ŸÓhÜÞõ?zQĘ˾Z? €­"—4?ïC9Û×?§L·fv;?
IüC?`KwÖ-ý?Éð÷€C?Á­o	€»?é?z0ó"?Áá$®Z5?¥ÁÎÔÕS?œðÆ×3eÛ?¥×I«Ú3Ê?ž,¶jj?íFnw¾
Ó?¥Xì¦íü.?ŠVS¶ÅÖ7?q¨ÚîèDf?¶Í‹Ù½v?áyv¶Q?ì¼õ5Ãþ"?Ÿ…z&,|š?"™ñw3å¡?£ÅÖï/?x]1^ÉÆQ?xéÊñ—½º?ï*vÃæŽ?¤k¯ÁÃ?‡ütÜÖ??–b'ÇBt?įõ·¸Ï¦?óEú?êt¾>>ª?Ã	ör|c?£[möéÛð?˜;æIÆS©?ža3ëw¯O?—6m<}æ‰?í×?lž†?¡3´+xü?rý<î~;…?b'Õº{v?ºd,"!?¥³ÏÿL?ìˆdúãä?¥XXWOTHER4FGL J1109.8+4406¿ïÿ¸R@O»\6À:À@æzýÀ<±*_Oð@WŸ
ÌÇC@ñ¦Ö˜þi?Äá~_¬bõ?°¥¸¶ÀF?ä»[áF×?ù¹99²~B?ì‡À=È7'¿ç"y߿éÅEŸFÅ¿î!çEôÖ׿ïÿµ¿Ö̯›Ž'SUNASNone?î­ã8Û$?Ä©zJ§v°?uºôS=°‹? W"Àc Ð?¢jmãÜ~‰?ÃFÉg±?íÆÂÉ!?°ú¼mZÖ£?žÒœ"= '?¦€Ž_ó"]?¤*¢OÎ? €I'Jcß?íëŽðâði?žÏ`§"ìÒ?‰ù	f‹C?ˆ7³(>–?ªÈɲ"?œµL—L?îv•2#51?Œw­èYeå?¡QpNáS[?‰Èu`e ?ò?b?oÇò:Ï®?ïS±Vñv?¯{†-2"?|&uU½?O¦át²?ŒË§¤BkÀ?¬í*´`N²?êÇ"aåßT?Àª8(̎?±BnÃåÅ?·®•âÒ^?¸"~.£_?²Tæ^âÚ?í÷KÑd·?¡Ûn­&ó?'?Œôê4?Žòxë ¹?³¨bbµQ½? gGþ?>?ëݶÌQÊ?«þdۈ
?»–HÊQÐá?©p»í?§E'þ—A?XݖèrAGN4FGL J1110.4-8023¿ïxz'9ËJÀ2aA…ÞÀ;k‰lû«ÝÀ<°±¤RZ@@!ŽUºF¸K?ó¹Ef;ž<?ÛÀÚ»¢ØÝ?éöh§‰Fe@"å$²fð@2¾/%1"¿ïÎ8<‡oË¿ísXHÕ\¿åš\!¾ì?ïgõbLM¿Ô1©ñb¿ïÿæŸÜ©ºUNASNone?ï_R¢S?""­Pò?`ÐÃÄO?uכ–ùž?'ññ\?'¨U?ïNٟnä?¡i'²øû?sT\ÉÁ?…6©áðˆY?'a7½Ó?¿¨ž…–Ì?í·õ}x¯G?¡üuÏŒ?…3&àùÜN?‡ŸââL‹«?¯3ÞlÆøƒ? v*PKø?îR¹­­š?™–$"4&?kZgÉu¦â?i¾HTÌmÔ?¬Å-äBHö?™9Tÿ[?îIÇÄ?ªŒ¦yÎc€?|îµ9d#?"0€3=°j?§Ê,å_l?©Ráé|K?îdÍñ O?·÷nôÅÞH?œLL?æÎ?§Eÿ½µ¹¨?§" •ÏT?³CÙ¥ä…Å?ì'Nð/ï?¨PÆãqŠ?ˆá¶F![?Šª¨Eëý?¸ÑQ²¶\Y?§~#ð•ÁØ?êv-fÉf?¶pEþâ«?ˆñ»ê]s§?'Ïßîëð#?Ę.¦lÌî?¶#ä·Q¨AGN4FGL J1111.4+0137¿á<Sy5X@K€`VìÕÀ;'‹®ŒÀ<bjáö)½@û}9f©@XdàTi?ÊÍG›õêR¿=ugÓQ_ê?˜ã#¶V5?ùðrƒÖ
é?ïîtÝw"â¿ëqBb{[¿è&Ï!»¼"¿ÔÈUÚ'(c¿ç–Háñ!@¿ïù&A³(·UNASNone?ï"ÎÔí`I?žŒ|P¾?P—NÉÌ?H¹Ñþ@Å?ˆùjLê]?žsê›)è?ï/ýD?–#íEXÈ?uú–öÝZ¤?zÅÄ
?<"?"¶ {æ?'Ú౒&?ïïA8P÷?‡20˜ÖØ?oSS=¯'ù?f^^É#Ëè?š—­n(JÏ?…¦Ì±>¾ç?îVçzÍüx?ƒãè¡Wf¹?…ž}<Œb?iNÔO~<¤?¥)éQl?Ík 
"T?ï2âTë·?˜L…i¶Òå?_8äݳ½?Uø¤Eáâç?—°'Ì7$?—àÍðMà?î§#^ß?©eÞ²üŒÆ?ƒkM(AZ›?ŠDþoj?ª
ºç8m?¦ŠÑåmö?íû³ÒÕÐW?—ÝŠ©™_?~£ö`=$?vûX±ãæ?¬pD	
n?–lò†?«¯?êû½²ÑÏ? %5]s½?ŸÃýÆ>é?ˆ¾
ÓrÍ5?ÀŒ(lÛ ?žRt‰BHAGN4FGL J1112.0+1021?Ô#?ò©€@N›‰
Z[–À:²˜ˆøa¦À<beÀN9I@ž¡@W@	z¾A?ÈlxÏ¿®•ûÝå©?×¥_ yˆ?ÿã&«esø¿ÝÏI~Ïø¿éu¢¿<_¿ïaß¹8›R¿ë"ãw3=D?ì.rýMž¿ïÿÒ³–šâUNASNone3FGL J1112.1+1034?ïáèùåE?®³ø®f«?…%˜bY]â?šGXÝ{k'?"pö¶uàf?«c)*£˜?ïžVå·L?ïjõp?fåäó¢‹?rŸYuð?'¿ñÐô>?‡ÌUD?íÇ;V©k/?žHÏÏ!?‡†hsã¥Í?‡ßþOei?­ª°t$à¢?›ÕÏè´?ïö¶I†?GšNY÷?8ÔÎâ?§-§óŒ?RSRà'z?Fd;`L§?îêòMÿ?¡t'â»ä'?ŒûV'?—BÔ§©Ö?"Y8¹+›"?"¥.<L<?ï1çƒ(áB?¢.îf5Ð-?o.SØHƸ?‡ÍÉ4ˆm?•ÝE!›ä?L9nª^?ìï?±V¶? Ó_¬ñŒ¶?"%4¯ïxG?¥'¶>÷?³¼¶È1:=?œ™+øÑÈ?ïÑÞY'š?rỹ?CÒk°4Ù?OÁcV¼À£?t–'®<²?pØ(åð;êAGN4FGL J1112.2-6055¿áVqKN'¿Õ8;SéÀ8¤à·e\{À:)1™Õÿ{@ 
y#ŒÈ@­'hr°!?ʚ_,
u?ÓOW xEŒ@T>S!æ?úyLò÷ÙÁ¿îg8¿d?¿ãÎ_ã¯+¿Ôv§ý	«z¿æ¿£ƒþ&â¿éR½g)/¿ï+4+€·KUNASNone3FGL J1111.9-6058?˜p7ì¥??"ûÖ~!?°Y)_Fwä?­¼™J°-?í1Yz?°ºj¤?Ž+? 7òÑíh¼?¦Å]}ð¬â?ÂqëӀΥ?·»ýô¯aN?ê`Þ*1?¹1µðí\?®ù6/ŽyZ?fV6"ß?ÃËß(¼Y/?«æ£o}³¬?étÒ\P/?¯'vÌ«Š?ŒÇ`lË\?m÷ùU&-?½Žn_{ˆ?›ëÉ0Bån?ëÛÐef??œWàýá`»?"îÝëC‹?yÓúNt\?°¨Ä¯YåÉ?¨ê`wJ,?혣®™Y?ª2<	½æ?ë›¸æb‹?–xIr!Ëü?Æ&Ó~lÂ?¿;[Ï«ò?éûGÜ/Õ?¿µ'S£?¨"j¬†Ò?•Édý"?Åö-fÿ?®X©û–®?èù.³?°.#¢Õð?jýE.î?U DqàŸ=?ÀÈö€œ¿á?¤Á
Ø®øé?ë²ÅH?¤¿Ö¾®OTHER4FGL J1114.6+1225¿çi¢Ñ%Ìî@O}Ëݹ"À;dÑ~uYÀ<›ç+ä<@g}ÕÃÁ`?ôFâ!ȧ¤?àþ'î?ïÿqÐ&ô@Ø®$kT@I§¾ËW?ï<m¿ ;à¿î»+à-§®?Òa¼­ž¿Ö‡KMÜ+å¿ïÿójÆGx?ä"e}2ZÆUNASNone?îÕI/ôºR?¥(àr;Ê?Žü×³ðò?'~·§1îÌ?•ØnwŸ!X?¡ Z¦Z@j?íz»/ôíÜ?µTULsÏ?¡~çv÷	?­*ÛàÈ?¦Õeø']=?§wd÷Œ¥&?ìe~åÁÃã?¤cs¾yÞú?¤ŽÛÛ ‰ª?˜:Q~…""?²ŒšæG]'? p§^?ê´+Bp_[?¨|¦¯+Ò?˜àôd$ô?ˆX"íË?–Öh#w?¨O±j±ÿ¶?í±©.Ѿh?ª^]ÀeæX?ŸÝû¯tˆy?žµJ:é€?¤öo;)ÕD?£;ú³,T?êLÁsA/?Ãõª©-Ø£?²	|–Ù"¿?ºo$>èaí?»wÏøÙÏ?¹ÿ3»³?êå.ª&Hƒ?©E/ªª?¥_ü Ý.?™‰Þ—xÍ´?¾&Œ¤Ç'Ð?¥¨¢èK#,?åHÁ÷u†¯?»äŽpƒ?š‹%'ªŸÎ?•ÔGš'JÂ?ÓÅɸÆ/¥?¼·¢:ŸZ›AGN4FGL J1115.1-6118¿ëˆñŒ}Z¿â-tw¡!MÀ8D~ïÊ'×À:
ž¿s@ rHqß@Öº;А§?³¾R`Ÿýâ?ª‹~g¨Ê?ùãòhgÈf@"³U?ìŠ@Ë¢*b¿ãÆ
`:Ó;¿ẩæž/+¿ç'¼£n¿ä˜êýºU|¿à5몥çUNASNone1FGL J1115.2-6124c?Ævæ"ò?µÒâ)'…?¤o6ÇüÔ3?¥	í/ƒÚ?é…™©×!?¹«;uª"¬?¸׌$ƒF?¹*ÝÆ#£9?£IR<º?ŸG꾯'?ëà }ÆKÌ?»Obu¸`Q?ĺÌ0çöÁ?¬û°VrÉ
?·ô[d?¤•Tèm?çߎhcÏ?±‹þÓ|‹¹?ÆB—½¡?Ÿç¦LBiU?­ ª/?‡"-ÒK;é?è•Om¯
¨?¡7†Ë}ð°?½•K8/ß?¯jluw?¢7YЯD!?›¡}àøË%?ë)àü&#"?²ªöf¸Á‰?©ÚD"9?§ëÁÉR]µ? ÊÂ@ã½-?£!F`\m?íaf:$Fº?°ç8ñ©Ÿ?ºˆôþ´?£ûÙϛ‡{?³u8¢í?¢ó×V'O?êN'Í[¼?«ŽD9'M?®;Ñs"…?'ac"‹?³EaK.?•2½cð?ë¹;Ñ£‡?œžÁz÷iOTHER4FGL J1119.9-1007?Ü:tw˜ŠG@GQµc#»ÇÀ:ë浬×À<b¢Œ‡b@N-ۅw?ÿX×1ª?Ñ+û›í0ð?΁ûWϟ»?üöË #÷@	^0;;X?¼äaئä¿ëY:>b¹¿Ã;Û"zÿ%¿á¦ßîÁ¿èRàýÜ9Q¿ïÛ`í*»UNASNone?ïæ€QQµ?^ûBògç?Fèa¨/ºs?B™Dð'?d'gfÛE$?X ÅÿmO?ïÎ;"Ö'G?r	îP‹á?I‡V¢®S+?PŒiZ¹–Y?u±J¾QÎA?n¡S‹9!é?R?{Ȧ|Ÿñt?cN¥JO?gôÍʉ2½?‡f¯*ˆ;d?x  §àn<?ïyôœ¹Mƒ?eèÆ8Å)¦?c£Òˆ¬æ?C'	ÕA?Œ™ä*'?dCíó¿|?ï¹Þ­—IÖ?wý:»Î?WUáì>6,?REҞÓ'J?};0ÕxSŒ?uÝjcê¤?ï\äڋ?«ªµ˜=?^!R§îú%?cÖ9Ìí›?'™ù-?\×óü¤q?ï'wØv±?ˆ<n^92?m,j‡¬^?lì¡T-e?—nŸ`|_?†®½ÔG¦™?î§F³÷ˆ?ƒ°S¡ëH?qc%þeè?\Ž
Æâºæ?£_0·|?'Á¸'•_ìAGN4FGL J1120.0-2204?ïûÅØ´.@B(ÂzÀ8Ígi›¥
À<ø¨ê@Þ}˜19´?üæ+ÈÛ¦"?«µÊ|»gu?Þäµ—&"@/êjP
@•'æxðW?ïùÙ?¡Ö¿¶UŒ_°zî¿Ý£¦ï¿è"kdÒè¿ïÿûbâMh¿ïæó{?UNASNone3FGL J1119.9-2204?«z9…qi[?±h²§Ë ?íQZÄ$eC?¸ˆú¤°Ö?žà4rHRò?¤ë:Xèæ?š?O¾\±,?§rŽÑŠ8ã?í¿KMV?²Ä«\÷¨?¦ë£Oñr?§&N¢"-ä?¹'çþì?§BËJ^?瞻EL ¦?´džräV?Ľ	ؓKï?²_¾#v-­?€Ó_éj¬b?pà]PlB?î­¦;@?‰²Z‡jTù? ðÆÅõî?…¿ß®šÀ]?¤ûõG?ª´²ôßf?í¶G "¹Ð?¶CyråÐ? ƒ'ìã4ò?¦qƒ}‡ñû?'#ºë­?¦zÿÒí!?îUú¸ÃU€?±²¬êH!œ?¢vúÙ²?¦NùM¹e?³j¬V–¬Ù?¤ä?ÍMå·?écK¶?´9¤¿Ç?Â=¡=Ÿ??±gþÐó&?eºä8'P?\{K~šA
?Æ9F?"F€f˜?¥ìA)¿7?'ŒcYPSR4FGL J1120.1-2645¿è}w$#Ì@?Ï>$þ½
À:GXS~,VÀ<_'fÅ0÷@÷´Lù,ý?þèõÝgNÄ?º/÷¿i·Õ?ƒlßHǼd?ÊaÁ'ýö@­¨ñ{Wå¿Ù‹Q¢Š$¿ã5æzyC¿Ü팈†w¿ßœ7£Û;û¿â6þ™Îs¿«P'	ÚoUNASNone3FGL J1119.8-2647?ïëӔ«âá?N½í¶õhÑ?=÷ •¡Ê?+ÿB«šr?`mw0Éۆ?JqâûŽ¢Ò?ïßD÷´?mŽåD.Ú??wÍŽ?I0¶BÜÐ+?lÍI×ʍ?iagvG?ïµ¹ÓÔ[•?o¨'Û\?QÄKÂ?H…s…Õ_Í?€Y	
/£Æ?m¨¾À¼"…?ï§j€¼?^å¦9D',?P¶Yïc¾T?032ú;G?""	·N?]䝬Êã?ïÛTŒÊ(X?`Êì=Ñä?JË{/º`?9ˆ &dc?mø"w­øØ?]ïÁ$•9!?ïŸÒæ
ÝÜ?"mò0½lÇ?OT"í¹]?Z"	âySË?†Uv…?'ä@GŸý
?ït¤nMªG?~N;½¿jn?[3ÜPxhr?Që'«ä?phî7?|òý ùŽ?ï{y·À»?}ÇÓ
®õ?enöÇ3é?M®wötœÈ?"±ðMf'?|æï7+Í{AGN4FGL J1122.0-0231?ì.·+¶ù7@J¬wFˆzÀ:õQ³PúÄÀ<Cb?8È@Šx•½ìà@c줩(?½É¹ÇâWN¿»é\`º;6@k:á}]ú@ܨX¤0÷¿å•b'¬K¿å6fœí¿èð«Ï&C¿åé'yâ¿äû9âyÝ<?Ö¶›Ø'UNASNone?ï´DÑHæ?~r
2»è?[Wu1ƒN_?Qpg_úU?º Z8?|KúÞ¨O?ï.뿉{?ßI±aÒÒ?}nοÁ œ?eðg	83?'ÆÔmވj?'ÉMîË?ʺ¬?,=WNp?tгG#ÚÃ?u¬úãUŽ?š8Ü3ÛÄ?‰û¥
7§¼?îÛÔzsÂ"?ƒœ"›†®?s¦^½?bãUŽH â?Ÿ›ëf<‹Q?ÍÂÆܙY?ïZr捤T?}84ÛÇ?q >ͼÕ?e¤ší?R¸?n› ÿÀD?Ž†yï>È?íèèÌ)0G?±"Ë> Yä?ŽÌÜÉ{?Ÿ¤&í(¿?ª
ÀÎm§?©XaRї?íôñ2vŽ–?–ä©´Û´?†Iaë#òE?''º¤û{?«"[:e?"Z@'h?뢌Î@PŽ?¦ÄjJ|?'iƒÂ»Ó‹?ˆè\ä÷)Ü?¾Q8›–¸­?¤w®ÔAGN4FGL J1122.2+3926¿äçaââҌ@PðváÞ¬ÉÀ;(à#Á¦(À<'i<Ú{â@#³—œ"@[iQ;?Çúj"2°¿¡C!£ú׳?ÖQå&µÌ?ü¾#çÈe?Ö_#Æ®¦¿é¢²G‰
¿çXl"h	Õ¿åþ‰¾]¿éPKý"z¤¿ÓUG¥[ÕUNASNone?ïÇè6q?qr¤_â½÷?W
:D,QX?KJÝbÀ˜?v¶©ál—Z?o<×æ8E?ïK©eƒVP?•Ar7Ü?r¦ ¸t· ?yWH{˜Ìp?'áK@Ú!?'…ŽyôÆc?ï;–#²?‰Íú ð?xkvTãt?x"ËOªÓJ?–¿ù<²Ý?…5__w&?ï`Hª"¼á?p‡MàµAS?væ
Í6ï?_gU‰Í
?ŒzÊPº\?iÜ?úøtg?ïEåT$'Ò?'÷ÅdqÆ?iïþ~kX?`ÑH$7?"Wuš§Z?DÙæË,?îG©šB¶ß?®e+ÓÃa?WÅJùT?ŽZC€Mç@?§/£.3h9?«Jd6½)·?î7O½WŽÝ?—Âþãbtñ?…K´A7C=?sb:H?§8¨ÝY?"vQQ<™Ê?íÛ{ùm>?'	Û«u™?'{{`Jò?€ÄÀÃbîr?©
'Ú£?¯?5Sï¢WAGN4FGL J1122.4-6237¿ç¹]¤Jø¿ø"ÊL¿ÌÀ9SdžJÀ;
¸ÜU
@ 7~ä6¡@Z¨!ò™?¾ònGx? ÜñC_âO?æ)Ïqºû@I4ý7Σ?î²:zOQw?ïàß¤jٿ媚rÝm.¿èÇ)Š=D¿ÍÀ‡Y¦¿ë	c@—ëUNASNone?Ü}[ز£?Ƌ+Æò1?€­æ2œ†?vSÚ^
e?á!š¦×<?Ɔ6/¼Ü?ÝÖàMbp?Í'
Ÿ¯÷ï?£Õ¡Îl˜?‡¦ÿ×]?àΦ:‰5?ÌËÌkAÜ2?âé£xÑ´?µ¢j$kW?¦ÔIW?˜*ó:ùð?×kt05­?³´áh®?å¼Y6ŸpÀ?¨í²4ˆ?'¸âÒK%"?zí‹;6|´?Ók¿f\ÖE?¨f]ŒaÈ?ÒÊ6]<ϝ?À4fÏlå1?ÚaýúUí?ˆ"Ùy?æÁBb?Àsmº1ƒu?Ь݉¦?Å"rpéU?ƒØ§À³—Ò?žÜÜƒ-"?çZ.œm?ÅóK*?Õ߀÷®š?³žå%6¯å?±ð½"ÛG?¡­§€}Œõ?âÒc‡ŽÕ?´‰£Áá?ڐE'?²›ªÍRì}?¡MYÛ*Âþ?'~C²]Ã?á£XêìŒ?²¯#k*u"MIXED4FGL J1122.5-1440¿íÁНòl@Ezã`'À:‡ànj@æÀ<N&äpX@Þ2>k @|ÿŸ‡ð?Â|ãUzZå?°Bü>l?çu	Ar;1@ꖧ 볿ãOµqfu¿âøÈÔÈ(¿é=ß>ir4¿ìåþÌú6¿ÄçxŸ£ô¼¿Öԓj«o…UNASNone?î"%E"¸«?\Œ6É?ƒ[Qc¬›?¡ä
šÒn?¢æ×UŠø¡?¾ì"Êҙ?ïm-Ŷ0?—ýË¢tAm?jßa‡­R?rkЭ´Þ?üËÁT¶ ?–@ÔÞ•?î芋Ý?´GU.?ƒA €3?ƒ. Ú­?™N-˜;6?‡RõZ?ïV¬u-?olœibY8?_ˆ"Èè?N0™|W>ê?Œ9R_‡õ¹?l±02N'?î cƒ™8\?¶TÇaæÀb?‰ÁYöSA?ž­Ó}å	å?§‰qG.×s?±$í9ó¤z?î‡$Åd×#?¨fÝo1f)?yŸvÖµ©§?†ü£ßU«ý?¤YÄÑš?¥zc€Oh?íâ`"XÕ?—8Rñy?'ün˜<Œ?Œ––½˜½¬?©Sø"Ž¸v?'h±×ø?î&®ª:Y?'¹¤ã
/?}΋ƒG?tDVc©¾?©ÛE'}Ã?3âß ÉAGN4FGL J1123.2-5111?ïרcó@"š{9&À:¸ÕŸeæÀ<RÂ&@»¡iÍf@NeÙx¬º?θ©?Ñ&?×8´|sîå@·±ÚØÿ
?ü|h±D[¿ïuH¡¯g·?ïé$ò'Ð)¿àL"b¥¼"¿à2kݞ¬(¿é4èªxäî¿ïÿŒ	ß}UNASNone?ëW#¹~Í?³'	Š¤P…?C=™ä?…×
Mkß?Á®;½}/?²V­Z4?éÞ²8)š·?Á7¾CƒI?¨CÀ|ºï2?ªÓÿOŽ°?ÂtG*ÙY?¼yhƒ™t}?ì@Ï‰?¯?¢rÒU7?œŸŽ;œ­-?¬1n.~:?¶Ó-ôÎ×;?ž=KB§"!?ë?³‹LÂ?'=¯××>?°JëÝNÉ?ˆL²c©˜v?µ¸N·œYª?‰áù0Nx?äƕ_<r?ÀL±çø?¢Œø¿w'K?˜SB$ñ/?Ô!6*"W2?¾òCX36¨?ã›þÆ'l?Ë«5g.Ò?¾B[Uwfû?½;WÏÛÜ?Ñ7kŸ"â(?Çq߇JÈ·?è¥k~ ?¬¿îðr /?§}Ølïë«?•xêGh¹?nj
•8X?©V8¦!®?æÛOŒã±H?¥Ô"'Œ?»é¶|ÿ/ ?iiٖ'?Ɲæñ£O? Âøxý5ÙAGN4FGL J1123.8-4552¿²¶1¹bA&@,­kD¸ÃÀ:2ϾÕÀ<Hóµnâ6@Œ¾A™¨]@ÜOÜ·%œ?»Ýظ¾M?±g?Õ-'?õ/$*³Ê@qI^BÖi?ïùJYPԿʓÂjU%¿è-YŸ®†'¿à×ewS´¿áÙ[ñ˜^0¿ì"Áœm	UNASNone3FGL J1123.6-4558?•Ñt8?}¯ØՁ—¾?Zý´†dõ?K±9†æ?‹õ£éPQ?|
h3Uâ?Œ?"´e=k?]éQeð?c>Ƭҧ?Š—YPè˒?á¦KúAŠ?ïLBÌw?'‰L"x?jq®ÎöüÙ?c>ïTE?")p¦V!'?€¦;"`°n?ï)Ä·!`?jÌQAÓô?}fõ[¥?VKŸÿLñ\?"ÏYŒ;Í?gÊ®,Ø4?îó3ˆþ]?"Iµ.4@°?m+Ïh¿ÑL?a—âðZ²‡?ôýL£E?'H™¨±ZC?î¼,Ezªã?£…_†ˆ?ssg-œ'Œ?"¯/7Be?¡Îο3]?¡À›6?îX#–nR)?–Vk"xï,?},×*r)?tnS‡©?¦Ø+³^¨?"
ª†"q?í™áÅy¾ª?†<|³øÞ?•ƒO¢¡øZ?vúˆ`Nä?« ;Òǖ5?ƒ:X'ŽvAGN4FGL J1124.1-1203?ŠN÷`ÿ\@FºY!…ÆÀ;+Ÿ'xÀ<•®Ðbƒƒ@Vï|úýb?ÿ!ƒ†Ý?Ü­$ÜtÏ?ä¶öq@"恩¸Ì@ïZÎy¿ïü!~|?ïÜ^o÷ß ¿Ù€¬ã£S¿éCa(¹Þ¿î-‰Û¶tœ¿î¤Q]똕UNASNone?ï)<´ç'í?mÀ¼Œýn?"ný,G?zÏ«5
ÁU? êÑ«J?‰gYag?î§g»®Ÿï? óO,2ïß?$.›dn?'¹‰kQœP?šîÙîǔ?•A"O¯A?îWÈ7€Ž ?–õ(-#W?'&~ïÊ?‰aó´?¡yvy!?'v#U—!Ÿ?í+{=…i?¼2??¤¾(yƒÀ?‡â…rzƒÅ?©+ûÀP?…"§àª?î#»W?¾?¡OÁ>'D½?—>e½àP?Ð…¬h?¢ž'j¿õ ?š¡á¹.d‹?ìQ:Ëe?¶ÊtÝ2?¤ÛÇA–¤ý?©®סŸÊ?³FþÝ?¬<=8"Æü?ìØ>²j?£¢.ɯ'?Žñt÷ή?'ZÅë©~6?±ÛÑ®é?ŸûŽJ>?êqå&µÌ?¥+Jw·Ø?«mG€ä?Ÿ¸‰È	-?¾¸
Hx*?¡^}Ç}˜âAGN4FGL J1125.2+2557¿à…˜¦yk@Q­LD|0ÓÀ:+·=ïOÀ<€¼ÈrÊù@Ùÿ°yÛ@ð@|ÇÑ»?ÄàðZÆu?ÕÁ~gô@	¶§[ùûÚ@rZûÏ×?ïýË<©Ôz¿æ	g½~{0¿é–¹èîl¿ê""½¿ïý²GæHŸ¿ÓО¥2UNASNone?ï¡è[S?ÉèFöÄ?xä'Vê?*tŽ@vÈ?v'⠈F?t¹ 3ˆ…?íc Q!c[?³Âûɬµ??¥ñC¢â°ž?¬¹FyŠP>?£Ô·Nvµ³?Ÿ
ﺊr?í‹]mæ¯Ä?¡»æ—‰>?ž^©¿½«Ù?"÷Ï&e¼À?¨Ô@ÚFÐ?™6½Ð\X®?íæ%ÏقÏ?‹97x?¨¾ô<À_2?‰8'?Hšm?'½]'·áË?rYøºo?ïU/`¯‡?"Ö'¾÷·?…'R•|"?­í"µ·¯?…"Õ0ã;"?€Ålº³?ê»ێî?ÀMYò\ ?¹*ºµ¨Uæ?¾•£A§Ú?¶§lk
?.?°Ù`ks?ìòΛ¦[–?£[‰3]	!?Ÿ×¦l&I	?•¿ü¤Mÿ?°s¡ˆŸx
?ŸÂ'Ÿ Ÿ?çü¦×o½þ?­±a­Bk?È[¤Öä}Ã?¬ÖLU؟u?®Æÿ0áÅ?'ëçŸTý/AGN4FGL J1126.0-5007?j``@$ìܨââ¹À;E²à'|oÀ=–"TÛú@˜Õ1 6?ÿoB]r¡Þ?Ó|
}é?ïG}½›¢@ÇVO—î?ý)ºËÃ?ïû²}ì¿æ5‰2C¿È'MÅ°£Ì¿ÒՖŸê³¿ïþÂ^§U¿æU/þËMUNASNone3FGL J1126.8-5001?֊µgͼ?ÈùÌ ÷¾µ?Ùu&?&Rò?ǹP½¡z}?Ð$Yñ?Çð*àSg[?ŁÑÞ¦áM?Å"¡ô"?ãJ¥¸\É?É·°ñO
.?ÍS—AO«?Âp—Æõa/?Ú¢"ð?´1¾g†?Û||_C~Ò?µŠŽWfÜ=?ÃÁß;—ä@?§C¡7?Ò1#1 è?±‡Ž3.â‰?ä&MÏÁ?´ZOVg[R?¶	
Tg—[? &UK®K¥?ÑH¥Ï?ÃÜ[é"`?Þ\èU`Ñô?Ʋ½äÉæ
?ДÏŠ~I?Æ)˜]b?¯
ùj?¶aѱÄûË?çOd©?É:œ«iG9?Ë®Rۑƒ?Å5
p=Í?ÔC
¬ø?´Ì'?®îJ?à(›÷å!?¸Ê1û-eò?ů'
?«€õ9Ѩ—?´ïíîmvõ?¤Œ8CNš~?éÐ[j3ûZ?µˆuÊ{q?¼6Áª|7?­Ý,Éë#®PSR4FGL J1127.9-6158¿Û;_¾Ú.¿åÁ¹óêHÀ8ÿÁõuüÀ:²ÿ%¿­@Òg°"[<@–øAŝ.?ÁÇHhújj?֚ɚh@ߧÃ(]?þk§ùÈ.?ãů¢›¿Û–­@•ql¿ã×ómJ†¿éå9àÌ^¿ì¼í[¸{¿ïòÌ&°nUNASNone?¨OÉ"£?ž'¡œ¬ÐV?҉´¬å?ÃFt°£mÐ?å:­Wš#?ÄNçf"–$?»6õh*?µZ/OG%?ÃôVǒ?³SÙÅ#x:?ç"ÎÈÙ?¹S56až¨?¼°§µ«'?£Íþb1}š?ÐĤñLÅ?±L¾ª-G?䘐/7¦?²Ä"øµA?«d
>َå?…¯| ]¯¾?ÊÎ(úAœz?›<ӔüD?ç–4í|Ó?ž€ÓîâÈÎ?£TÇà,d³? lùœª?ÐZ¤=ƒæv?ÂeÐý'™N?æac-ˆ
?Ã}®®¡
?žˆ—ÿë§?œÔ#0ÆAN?Öܹ1˜?¸)[-…?ê*4aŽ!?¸/Î<Ît?°Îu3¸ç?–-ؘlyÏ?҅ž<£Ó?·›íʲæÿ?ä£b]ö³Ú?·ª¯ÅÄ´"?ŠüÒ°ë?nøÓ!5ëÛ?ÏËoŠQ} ?§$'Š¶Ç?ç¡0Ò¹S|?§ˆî	_.¢OTHER4FGL J1129.1-5230?ÂüÖ#|u¶@ ´Ž:!dÀ:ËêpKÂvÀ<BW¿¶n@/§J\D¤@#Êŋì?ÁÊZÒbä¿¢E›ÚUe?áKÌQ|ÊV@
ájCÒ ?é|=}¹ê¿ÃJ&¿²]
¿ê……t¿Ù-Aª‹¿ßEqcÅwC¿ãñ" Ü.UNASNone?ï¨oCjôý?|	Dš·Bv?Es)Æ·i?;SÄ>©AN?"Œü'ÜAý?{°'T¿?í¥‰'n	Ñ?±äÖl©c¡?WÐíÛr§q?fuµ''Uÿ?²to³ÂÙ?±´ûðˆ?îç	vBÉÌ?x5ãë!?i7Ò[*?eØ ´ö­I?Ÿî°Îô­,?CàJE-
?ïºnîË$V?\šœLG}?D£ÜJ?)sÆTw(C?€‡Ê·c?\óeßv&?ïo %ܪÞ?ƒ¤¬(¬?U˜JlõŸ?I¬+EŸ?Â{?ãñ?'ë…b©Ž?ê(;éM¦?Ãá
'©`6?j/)cÔÒ?€ÇàÏB-Ü?ÆöS·jÃv?Ãtü+£â?íœ0 ?vÊ?…Ϫ{'ä?t²}Û=ùï?q!ª?±ÓW!"G?œ®õpµ÷?ï	Q@%?{ôJb‡.?aº—	¾?O 'ó"|?š‡'ùk§ž?{da†¡AGN4FGL J1130.5+1400?ÏŒBn¦@PÁå!WhÀ:È£öꭈÀ<r5r
	@a
þw¥@îùûA?Äm¦ß'm?jF/Ä{µý? ÕÇóE:@ýClç4¿å¾¬#¿æƒŠT'¿åGxÏõv9¿è|üÀZxœ¿éÒŠÝ>4¿ïmè jUNASNone?ïçPðn£³?`Ür‡àø?Cùw¢¢ã?8iXŽ'?c°±¯)>¹?\™!ÞNåÎ?ïÙ©mì?r=´"
gî?AäÑ[ïª?K®Ö•ï;?q5'ÀF;?pLwu¬þD?ïˆÛëƧ?€À2'Já?[w=p›@?`FÕAZ|D?ŠZWÔ¨8?€-ÖjÃâÕ?ïÓ²xÒh‡?S"§µ†?TøÂvkþ?<"ü?û¸?pè".v¬?Pç:ÑSˆ?ï¼G½ó"á?vÖnRVH?TiLGå?Il3·\ö?|Ú¾*ˆ˜?uP½B¥Eç?ï~ÕÖ`ÊE?'±&ÒGx?TUu´U?aLÉQV+?¿è|št$?ô/‰§Ök?ï¢J"H??ìMGeØ?g<ýDÜÀ?dóÜUãë?œÇèz?lI3¸"º?ï|ÑÁm?t.+ؽ>?nëά?[ý)–9X_?‰F‰"ê?î?qPgµ±AGN4FGL J1132.1-1448?ëMߏzº@EgÀ:÷nªØ†>À<ræY¶U@ #3ºÂ‰'@¸ù±1f?ÐB¬©—?¼¶ðÂuZö?ñ åRՏê@3¹ˆw]Z?¤àA@{?ÒD4¢Éî÷¿å.â q¶¿Ñ²;{+¿ßö'þ¢ˆ¿ïþù:!EUNASNone?ïÜŘŽN?kü%TI@?>­G­?6ØX³€¹?ob%ê؁?hù]i5?ïÝáà¸ÅŒ?m™**h?@Ï­Ò^¥³?IfC/LJ?mê3òï÷?h³߯Hõ?ï¤ß:šˆ?tž=ÑEz,?V	GšOú?^8Ýk$l?"p7Ŝ?ssL°_<?Éïç?eæª!.×b?a¢~µÇˆ?CLUÍÕ{É?ˆÑ2j¾îE?e$]—?ï¹à݌ì?x4ï­ð¼2?HäÛvI&	?Cž·ÿø×?òõ³§^?v™I	*Ão?ï'÷Oh"4?‡I0¦Íu?RÆ]WÏ?[|pü²ç ?‰)kF:›?…†Æ܇z¿?ïRO
Œä?"Áüáƒ?\º%ä>Ñ?VlZ¬à?"ê{é˜P?"xºE,?îÂXžÁe?'.[߶À?sޙRGݧ?a´ˆ¸>m?¡^¢ë°pS?ŸÂêAGN4FGL J1138.4-3555¿å(ìD%7·@8¥à?pXÀ:Ì<Ý ·À<{(7V®b@ؽ›×a@Bý@27?ÐâÛ¬äz?Ó(.rýN@ä%C†gŽ@`'ÿ÷q'¿åív% Jù?ïý»ýœ£d¿âRÞt?¿âw8¡Jr¿ïú?–më¿ïÔ. §TîUNASNone?ï"°e…b? 1œklEà?tÎvÁ‰'?ŸÓ0T‹¼o?"—XP µ?yÕ›j˜ê?ïˆƌtv?‰—Y¦ÙÜ?q~¶ƒ7Â?wt"cò‹«?…@E¡Fµ?€ =žg?îùÓWDNR?ÎGຠ•?'Ó«)Œ/í?€YÁ²Ã?—[¿PE¿?‰»A–­K?A2FÇ?z³Þö7WÅ?'T(j:-?p#×ÚG®?˜™ot¤d?rÅkàõâé?îÛ0úìX?"dŒ‹Wü/?‰fƪìÄ?…ÂÍM-ãÇ?—æ}UžË?Œd›mÖ³†?î£Æ bá?¨ÞCaÿy?†j©èc?'óë)?V? 3ÉO!¢Ó?¤@*!¦?î;ΜÓg?˜öò\ ·=?;$+?‰M:…ñ~?¤@¡Â»…?"‡­ñ°Õø?ìîí˜
AK?"xÃCÒâ?¢D‡<¡{M?‰{îuÚpÑ?®ÌŸ?ö»?ŽÕ2õUAGN4FGL J1139.2-6247?ëÇY5¸¿ñt¢iKôÀ8†8<‡oËÀ:¿mã2ià@uòœj.r@¸*Ž;?²î	!U©ï?È3<mn˜d@þ¼ž_ç?üQº¥WèÊ¿î¬B®Ûö?ì"ß(#½¿â†¢F†¿áë,i–¿éH§8¾o¿ïþç àö%UNASNone?°æ—ÇYÛ?¨[ӟ֞?Ú}3Š¤'Î?ÅKoËñ8?ओAT¢Þ?Å ·–ÀÝg?¹'ôr ^ï?¸ڃïŽC?Ö½Ø4¬Q?ÂRü"Ä%?áÀ…v!?ºSQÐq?ǔ(@!?­Šßã Š?Ôgûj!ºn?³Þàø2>1?ßÍö†7DÃ?´5ÜÉ®°
?¼ÛҗD³A?—c	™ï›?ѲA›«Â'?¦qûÀ·2	?ã‹dßAˆO?ªï"MŒï ?¦Å'»›û]?©í"=p@2?ßxkÒóÃ?Å#îWóK?Ý®áõ}ðò?ħLpØ'?Ÿpp'ž´?¥€~†ìä\?ÚÎí&<2i?ȫۊ¶õ?áèTñ'?Èw	™/?ÀÿoÓ2Ó£?¦ôمXI?Ö>(`¬?¶–Ás˜Í?ࡼ'õ
?¶·S'Ô?¦¹â%®Î%?ŠÂ¬p2ƒe?ÔçS	×)?´¾haçq?ä ¸XS¹?µ/òu£§,MIXED4FGL J1146.0-0638?àŸÿ¾D@JZ?>pÎÀ:b=ç™À<M·½q7@!'Æ¿¬?ùð'Iü?½³TUª?½`OKÔ®?ý\ÄÞÁÂ?þï·]yÙ¿ïý?Æ¿l'?ïAJ·æ¿´|£ÿùõп;«·ShÞ¿Ø-‹¾åƒ}¿ÜŠ"¾@BUNASNone3FGL J1146.1-0640?ïå­ˆ'Æ?{2`eËÓ?Q†PÍ´¡?AOµðöKn?†UʎŽ`œ?z	m{QY¸?ï¶ýšA¢?€Üþ_ú6?\Ò%ÔáP`?eËÿáaÛC?}L©rEêà?wú\WçÄ?ïHX·"Ä©?'ç3Ø®5?e9Ã`£W?^Ë»¥j?"M°­Ÿox?'6· ž?íׄG8o?ƒ½šÀa4È?Œ`×RÈá?mH«;ÙÞ?«oµ_"×?=Íá4æÏ?ïB6e­?Ž¡Ió0g;?d¡.fš?X`ÃÈ?ìù?•%~Úç?<Y˜9Ø?ï´î–?˜¢y:t2;?qù}Ììò?y_éènk?˜+ð3¤à?"z[MÊv?î†Û‹xæé?"…RŸ;y?p~UaV•7?eæÙå m?¥'|˜=4O?'µÆBfyS?녮¼Q»›?›"žx"Ÿ?˜Íà.d¨‡?'϶b-kÑ?½Ÿþº†?™|>³Ò§AGN4FGL J1146.0-6822¿¯IMñfÿÀ
[>ê÷ZÀ:lF"
qÀ;Àê×yÎù@¾§ðõK@W^ FÇe?ØÖrÓ\3?Õ'H㞠@¿ìTR@ã´2!:b¿ïûì?XÛc?ïÿ©Î›&¿è0Ç}Øró¿â±ŸŒ¨¿ï䍞8º²¿ïÉ™"{UUNASNone?âS³á™b'?ÄXnr	Ãß?¡?ŒFš¥?™8Íq¥n@?Ù6ÐK²[?ÄUÿ!D¡?ã\ …œ?ÃÅwªÑ?˜•›ÒÕü?–jõŒ÷"7?×¾wœÀÉ?ÂY"£?åbQ§Î¡Ê?±0…Bšed?´ô'žÃ^–?¢clùâá?ÏüxšÃK?­wƒÂˆIg?è4¹‰_Jú?œ/œÙG¸?¨ñKü?ŠúhѾ?ÈðÒÀS?™ºŒ	asP?ÚYVƾÉ]?Ä p–s§ö?¯é†e&ã?¨'kÓ‰?àÔ¼6keÃ?ÅûÔøy?Ցä9â
2?Åsƺþ²è?¥ÈŒøÖ¨ß?¨yÀSuP˜?ãڅ
9?Śh½ié?Þ渱6ï?³ý¦u<pˆ?Á‰ÁùùÅ?©öR4Þ·Ž?ÙsÔfQÌ.?³
Ž™‹Vá?á$¸q )?¬õĽ´«ï?±Hš(½?¢#", ¦?Ø«îӐi?¬Ðx
æ~MIXED4FGL J1147.7-6618?ÒV¨/Àê^ ŸGYÀ9ì¸ô¨´À;{oɼw@ÖÙ¶?A´@…æÿ}ú?ÌÞÏÄ#?Ò6Á}cX@-F|¼A@ç;¸è¿?椔3ÿ
?êÉTýÞ<·¿å'ÊÞ
6æ¿èæRkÞ¿í¡]¹»¿ïüL·h·yUNASNone	?Ýx¦zŸü?ÁI
B¼EÊ? è_¯¥åü?•|ÙAÄã?à5±ã΂?Á'ádgc?×ú	ý?Àڃě%
?³·
_[?¨¿»úêì?጖O†?ÀZå(D?ßÉ`,v¼±?²¹ivCܬ?²-¤½üK?šSƷƬ?Û«6¥®[?²ô£(Ú,?ß@]´wQ¬?¢ÉQŒÿ?ÉK¨•5ñ? Ýl×ÓÆ?ÔÎî+[? Xoüðµ?Æg&"r?³@Álz?°ôзh­?¥Ð§AµÈr?è^L!IYn?¸Q¢º‹žÞ?Ä`k¥•{R?¹ÅݚOw?»ìg9þ‡
?·bƱN?çjX/ZÐJ?ÁrS¨QK?Í)±kê¬(?¯L5eÕp?¹3Ðêp?¡Û"yð?å0jèˆ?²xÖ?ÍëŸ?£?…OUk?ÒÄDØ÷þ?°²œŽÀ?ÞFz·šû2?¬~?ï*ÛüMIXED4FGL J1148.2-0029?ɛ»žãA@M<=îx@À;+&ø'MuÀ<‡·ôÎs–@֛3w¦«@BúP"–J?ÆHàÙôþo¿˜à>ˆk?Ñt¶`NÊ=@€èÚ™ô?Æâ=¢Lñu¿Ý"PÄé~‰¿ßÃ!R`¿çúy
2ª¿á\ ý¦‰l¿ïÿå]½JyUNASNone?ï³	aþwÀ?vzЇ•«»?[]½f¥•ï?T7»*Õjý?£ß†ÎfÜ?t‹÷L¨¬?ï¡ eÏ?®åI³?YbÚâq?[$gT)MX?"™K‹±³ô?|²…Ê–þë?ïB›_[I?'jŒ)[Pƒ?v9-Í0ˆ~?wQ@팇!?'Hš—~3?z«Š%<r?ï\Ý@ów?m'5'ͼP?móÍؓ'?TñËs)B?¥ÞBãKâ?j'¼~9"?ï3<UÏH?'a¤ýÔ@Y?l¢`š?aHf–Ä?–^Q?¤Á0º?îû)/ò?›à!µÜ?j5ÿvYVë?t6l×yc?XžGk]ù?™"À:‰?îª<­8š?Ž'ƒ… ?€ã:t'?}ÖÊ£!?¡#f®È?ˆ­ñ¹lýí?îuuçô?‹éãkÇ9À?"2emñ?s­™¶þ?©ñ¢w‹?‰œn[œAGN4FGL J1150.1-6324?属SpH¿õy€TN5îÀ9·Lz,	À:öðf/	@:Ïzüö`@_¤?åÉ?φbЋž?³Ì{O,8?ð_zNz·V?úH'ëÕ|¿îóÑôSúS?îc2Õ?b¿ãå˜u­+G¿ìbXŸÔF>¿ÛÈFøã¿Ò…(€nzUNASNone?߸"–Z(?ȁÖ\?u.Î#?mé÷Í?ßòÀÀÀÓ?È~@ú¾o?ڊ'ƪ…
?ȗ…"ܶ?"['à¸s?•®·Œý?ââ
{¾'?ÇáóŒîÕ?×jÇz[;?³U»Ztð·?¨W¡_]I?—…BélgH?âÅ"`Ÿtq?³oN0\?ß°¶<x½g?ª±ã ýú¸?š?eó.HX?ƒßvçÌ?Þ«SdoÚó?ª`H–Ñûü?Ïn&;Ì?¿\aóÏ??|C~Qa
?s ¿³v?çëöùúŠÿ?¿±¶ËC?Æw^"*·?À',	`
?˜pY˜ób€?¢³çA¥äA?鞥Ž‰4?Àu‹Fÿe?È®ÄÛß×?«/²Ý?­ek´A?›H ¶L?çýþbhwZ?­ÐH»ÝE©?Î;àÛv4?«n"
ð#V?¡våÕ%n¡?"õb€bN?çY™k÷Iù?¬nKî-)5MIXED4FGL J1150.7-4613¿ïñVÁ¥Ô@.ºp6ÉÁÀ:†Æ÷ µîÀ<i´g{9\@›Ö_ȓ@"i7Ñþ?Â&Œš?¸[GàzÏ?÷êg²–À¡?ú%[Øï?ïôÿ¼
aè¿åÊsbοãîð®Se¿Ýñ^|¿åƒ^)+¿ïÿÅbu@UNASNone?îâ[¤bí­?«3çS¯×(?qME:']?•B²#°¡?ŸaFâ ü?§¶£}%Î?íý/ãiê?².t'iï?'Cz<×Ø·?'åÐòþ
?­Îoåñ*?°]«' ›¯?î£#$a"?•ÆH~gòª?t1g¼‰×?rÒïdF"?£G ¾×	Ê?•	òà\Œ?ì¸Âæ]ÜC?Šæ
OS<? vþ
†?z-<$N¸þ?²2-¿Iå#?…Ý{
û
?îC
˒ ?¥>ÒU{FB?fÐè?‰¿6˜4Ã?§îö÷Èk?£F{A?éí‡Þ±&?ÂQ±õS:?¦(¡Ulò[?§ç3ßz<?ÂÁ¹Šó?À††¿—?í3€NÞ¤? íkŽ$¬?ƒ]¨T*û/?}K–§"èT?±Š®ôcƒw?ŸãÐÍÌ÷Ì?çrlŌLæ?¡^û‡!&?´˜þ™A'Ä?•2g}—Ï?Çé͝›ö…?žI(¥~AGN4FGL J1150.8-1905?âÄÅö2f@DÁâCV—À;Çj
_ÕSÀ<Ýû@ý @"B;ë¾'?õò…=Ân?Ùõð"?Þ¥*ÜÍuê@Ðkæ'ø?ù	E0‹¹¿ïÿ+YJ1?ï)·¿Ža¿ï±	b¦é?ïþmÄ(¹]¿å¥;X›¢ˆ¿ÚD÷€Õ}uUNASNone?ï†C©«"?Š=X@?ZZbϾ{Ê?Sg¬ŸvK?‹#ÉDdÃ?‰3Öe4´©?ïW~¶-<é?ž,ȯŸD?~ƒ"/Ø;g?•oë漎Æ?ŠÞdSÌ?‰Õh1)´(?îD¾Žµc?š›"gøÚ?}Çjß³3"?€°ž\*Z?§û)Å_ëÚ?˜~(eT©?í×Û¾N§$?›jlŒCf?–j¥
Gú?''X†Ð?§Lñ''bÁ?"Pþ'#õ?ïm'H™L?‹kÄl¡'?i|Âì")?h/Šér	?ŽZE°^87?‰Orkó½?íßÐ2÷"?·œ‹Úqٕ?˜ñž?®b'vÕXé?¦tŠ?«¿z ë?í‰`Y›ò? ¬Cò††?ÜÍ¡?ð¯¥~
?±yc"s×?Ÿö ïhø?ê-Yúiµs?·†5˜ f?°9;¯Þ?²ÓŠ6M?¾[õ¸›_?°€\öiîAGN4FGL J1153.7+1857¿îAÞÀ¦_@R›ÓíR~RÀ;QÓq+¼FÀ<¦?|ÑÔ@\GŠ®@²9{Kй?Òx‰éù-~?Ãyç!·µ¹?ñJÀ²¤@Gz½áM¿ïÿ*LÚ¤&?ïâ¤.™p¿á¯ÊÈæŽ?¿âzó¼$ÞÝ¿ë6#það5¿ïÍ	žs`UNASNone?ߚãN?{1´ø)¥Ë?kmêÙ?aî42X'?'Â
X9œ>?vÜB=??ïÊ÷˜…ûá?wyqO]iG?NÄÛ.^-?U_+pg?v«˜]N µ?tf¤¨'ú?îægdW?'ÔãŽÞ"E?z3®YúZ??|Ñ-5d?œ±Ÿ("Œ?äx~ۗ?ïUsÞZO?p'¿Š€a?{ƒºOv˜?`>_
J?Œá+UM¢;?j£hҵţ?îáWÈ,ÃÇ?•'·k…˜?'ßMh·ª?yùƒ…U?še`DìH?'2=Zwœ?ï^ÿz|¦w?'Ðù?b®¬YôjÜ?pÏGò¤?'Ê;"ý¾?
ØPW"?íÛzõ"—&?ž2­Õ¥^?†çqe^XÅ?ƒtÏ\·x?¬ŽtJËBn?šØ~÷"ž?îfù†`¤?‹TÜä¨‡?‰Ëjâ ?w5"6à[/?£,é
½[T?‡•ßEb[AGN4FGL J1154.5-5952?ë']
¥¨ú@ÀµgUy¯À9ۅèÜÎÀ;gcRµ¯@íp¨‰¡@¶*ä°a?Ê«r«fÌ?ÞÅè¬ý#­@Â¥Fv@Ñ)÷öP?ïÿ«|,Ò¿ß¼ R:Š¿æ3ªïê¿í'›h¦²‡¿äϵù¿ïQ(l/ÔUNASNone?Þÿâ	0;˜?ĺ¦UOùÏ?€?÷6º?"aõÒ·B?ß(ôiý?Ä­E¢:kÐ?âøü¨Ý"U?Í5ˆ¾ç7?¯à½X[Mé?«Î‰w•?Öïy#z?ÊÌÂÞ-ë?ã£Ù«yã=?²…æýX8"?´/ž¹? öeÃxi?Ó¬ŒcXÈw?±,cɆ¤Ó?á‡B/)¯?¥\Ûmçt?»{ëoÒv?— u³ŽÌÝ?Ö€ÚŸ¸?¢ÊßõQ.?Ð0Rr"î?À߄Ól¼?¥¬³Ð(<? A3¬ãg?捊]ø•?Áç<;çÚ?ÐÓ¼Aܐ²?ËÎ ýڐ?ÀêYxtäa?¾>¦Ñ2«?ã[‹}îî?ÌQ¹'AZ?×ߖ%úC0?³E¨P4®…?»]‡MD_?¥Hàk%˜	?ऄZR‡?´þ¶â ?ÎK.sþ!?¥­rsÍÉ?ÈG^ÎÂpR?ªþ»ø¸9Í?âjU€²dc?­Ÿ¼šæÑMIXED4FGL J1155.2-1111?ÕOÇÿï @Hª›(ÂÀ;	)ÿ­ËÀ<ˆ‹y¢ƒ@!õäs2?øRñ>œ?ÜXiwÿk?ÔaæÕw–?ù‰,£Ìù@lƒ¼7©:?Æ5èDL‹?í•9î8W_¿âãeூº¿Ð`LpñÛ¿ÝÓ]ÀOâ¿æßÛÒú
xUNASNone3FGL J1155.3-1112?ï¨UëU4K?w°­q¿?\"
­2F²?O<u¬Õ=k?'fCÚ4[?tÁ¤n—‰à?ïÄ
¶vôÿ?wÐ䣞ü=?Qƒãüˌk?Y	"MŒg7?y˜+¥¶5™?sy‰ !Ó?ï"¿¦YØ?ªjµ#t?hоÔӊ¹?gó'ρ?™"P)c%¿?ZÜõ'Ü:?–ó³'?}¢:66µ?{_1$Ðmæ?eËAsq?£i­Z?|Yé	'HÕ?ïo"ÃW
Ü?"0ܳù?iüóσS?fÁ÷{µú—?¸K,ñr?±CHšôœ?ïGì WÁæ?'Ùo2íÜö?eÐÞ*Ëa9?p«L6ºQ?"H`'CL?vŽ¤œM?îã¹^— ?—^ù·Eä×?o"á`Àz¨?ir7µ"?¦–W.Ì?–}dX÷Ï?ìç±éd?—"š¸N¾?Uh†4²?{­y5y8?¶—Êp•Ù
?–€ƒ‹ÞfAGN4FGL J1157.7-6327¿¸Þ8P›§P¿óQÚ7ïZ–À8ô".E©À:•,oʓ7@>8?6¡¨@ÏKaþ!Ù?ɔš×1T·?֊MÌ;­U@áã!¢ç÷@÷ÚE±:?ìÚã{dû,?½ê2S¿ç×Tz«—É¿ëb)ösD¿îBýûÈä¿ðUNASNone?Ϲ½¢²Õ?ÁÌtݎw?Ս¯W¾OS?È0`eE?ڕqÖö"?Ʊ#CQ
?ÄhóÌã?½BîÅ£–P?Ãp>ÁÜ®Â?´­<ƒéÙù?æ	³\…´W?¾òqw®?ΩBO…Ï?°&(é0?È·­ÌŸ?­YŒf¤ð?â'Óûâ†j?³Áø	EáÒ?¸##DNx?»7'í?ÏkXáZñ? Àï¾Ò?å ؃¢•? þalBQ?Ê[k^{i?ÂɆËz?×?4'_Áå?ÈýÀ=Oõ>?ۓ¿b‰–?ÇàØÈ?¨ù£ã}?¦ÊÔù6Ð0?Æ,$ÖÏ5?¾þb="<]?èå\‹Ïµ?¿âÓIhª?Â7ÖjEª?§¦{‹XçŒ?ÎÙ	З?²aáÓaiç?ãìT µúp?µƒ5Á?—ýž"<Á?yɬÂMea?Óø"ѳ¼?©DUK_E?å´Å¿<k?¨"ì\pTOTHER4FGL J1158.8-1430?îº;h@G:‰ãC0×À;ÊNmK]À<}ª?K@!ˆ~7éPf?þ±ÞŸ]'ù?ÁŸ¡EŠx¿¿®å;µg?ïèÞ%d¾?í·«^×À‹?Ô}ÖÅt÷?|¹H­æ$.¿èqԞ}Y¿æ(ŠbÄñ¿Ê"Î×Ë®¿…Ôª'¹{aUNASNone?îЧf¥•??º;0¨"^?'ÆßøHˆ?¹Jç–èêY?"%Mݐ? á(vÝ%6?bdñi?¬,-ŪK?˜a}vâÛ?¡ŸÝ\´?ž'27¢¾?¡/(Êj?îËfš,«I?"1= :(?~ـ‡nç?'Õ ÄA?žÜ̔۩:?@ðíÔ?êŠìëÙµò?¤¸ZåS×C?š/x?‡ì6ç¡#!?ŽkpÄì·?¥Œ`¾4B?îÐT!u?ªì¯Zî?±‰'ó
?¨Î¾]?%0©$­Þ?–¸[Øl2ñ?ëÈìüÔ7¶?À±a­{"?©XՂE?¶âx¬¸P?µ0ìátª?²ÏDŒ"?íõ²@{è?›^'²yÍ<?‡í®OÑR?ˆ8DW,h'?ª³)Ksˆó?—~ÈÑÎ:÷?á
ì~?¶uÊée?°nL'¬tÐ?§O_¼7°?Ù´Q0i³?¸í™‰œAGN4FGL J1202.9+5818¿ï™ä[ùj@L×z_A®÷À;'bþÒÙVÀ<½·ªü˜l@(¶o\@HÿÚpú?ÄÙ»G¿1Y¿›Ï(¿`n?Ñs×þ")ñ@òà¦ÉX?ïøÀÛýÂ8¿ãÚ¥hõX¿éfòH‡X¿îQ•	ÖC?äp@¥½£¿êÚýç÷ËUNASNone?ïÚÅsY¿?—õÛl?\â…,
†'?‰_ù'†7®?fɧÁT?'Wf?æO?ï¤AVÁ‹?ŠË#Ž×G?`B®6@Ò?oé'‹6Ž?'ß9º¢"û?…4ΉüÌ?îቾô
?'*qC[—?rÞ°R'S¹?vÒԍQ]?Ÿ(	x?:çDÇ«?ïó
Ý^r?EÔ.P]?ñÜy6ƒB?`ÏÔb'?X;'ÃÈR#?DíSF‡?ïÓÔú~òà?s³Al?U'âoeÜZ?X6\0*3?pˊ=jH?p‰·&P†?ïI̼8?š
c¯r‹ó?b¸éî"?w6ç'ØëK?"o}d¥^-?–v8	"zâ?î…Á0Ȇ?–<jÛ Ë?ƒÎ{o{?ƒ
‰ìý–?©t&Ù©A?"‰¸3y>?ïÅÒªú?o8SûÃn?As´Y\*Ò?D«ø':kõ?zè†wÊ?mÃd"
UÈAGN4FGL J1203.4-6145¿Ùˆ#:Ò*?âé*ÁI¶ØÀ9ƒ×Ð6
ÙÀ:Ñ;§uû/@àúãe@Y~™cõ?ËPk'kSá?Ú=Z¾è]¢@½C^#¡Æ@VÒõÜ?ïÿ9œf¿äӟNå@¿åuWСm£¿êUŒáû2¿ïÿÕ%t.¿íýØ=CWnUNASNone?ÈñÀ¸‡?»ª¨":7'?ÁçkV¿?¼ù!'I?åÂtüx®?Ãݎ;¬j?»ŒS¾v¦X?¸ÎÇ?°tF?´Ú]´`?¬ýJ]»)ß?éó)Ñ=Ry?»q…֐'?Ò°JqNˆ?°œ‡íÚ‡?Ä8ه½›?¨žâçgï?áúÙ¤eiU?²…(}µ}õ?·'.ìöž?'hw±¿	©?ðÇé8=^?š".dz%?è!¨'À¨?Ÿ…7ÇH|¼?Àbn<Ò!?²Oð™?º-	M†›?µœ+0ý›C?è¹Æ:6‡¦?À"0ã'y?£ˆŠHZò?¤ùP…ËÓË?µa·[ö?±Ý¿‰'ex?ì#å¯5¦ð?´{Á[èO?Ä,óÚhý×?¦`r¸­|?ʝƒ'£	?­h¿{
d?åΛ§÷çi?²Y[Ò«â[?–"M7	dT?yƖÔϙì?Ç%²sŽ?¤qÍù@Ë?é‡dSDSJ?¤§]'‹6àOTHER4FGL J1203.5-1748¿ÖXþ¢'x@E˺Ü	€²À:d&°mñÀ<gÍ0ŸÚü@ý}}":7@…±ã<zÛ?Ȩ|¶^÷1?Ðӛ=]®‡@{ÜpêN@jlU\(¿î³zK¹?ïzV¨ƒAi¿âÍg'ߐõ¿âÁa~õÿK¿î'(]í¿ïÿ•AED®UNASNone3FGL J1203.9-1745?íˆ	ì½Øé?¢cBëC!Á?˜½•Q\S?Ž'ò,þr?« –ˆÏI?œ1`9p?ìÿÆ8!ô5?´$å>Õö?©?Úõ?­	e! lO?¦ÃÂcǍŽ? ]àׁí½?ìV0!A)|?¤G—ø'tø?¥z£o'QT?–¼)àzÞÖ?²'-=¿—õ?Ÿ>sÒ%J?ë5ÅDuÙT?•¡˜óTÁ?·™¦J¾%{?'xÏÇôŽ?­p_$ÝíÍ?ƒ È¬éƒ?èê'Ë2ݒ?·73%6êO?³Zêÿ=>?¥áez̓?¨CSoq[?²$°B
c?èæfPìׄ?Ä7•Fè`–?»ž¨Ñ^Ƥ?½{qv¡?½.$§:};?´¹åQn?èPº2{è?°rSï~C ?´Ä>û͛?¡¯2`™?ÄZ÷¹E"?ªæ#0ÂѲ?ç= 5ÄL?¨\ñ«¦?Ä(Kß¹?¦J´ß9CÀ?¾g財*?™Í˞{5AGN4FGL J1203.5-5745?ÔR"¢jÑ@"!Š"CÀ:˜Ž:À;Ö©n"óJ@aÎQ1@ ;êŠ?ÛÓuþ‰Þ;?àÈðÔéÑÀ@YcˆÕý?ü%͌Fµ?ïøÕ~Í"?Þ0×Cÿ¿çcvÇÝyÿé·R²T{'¿ïýðƧÞ?ïâÆ3U—âUNASNone?å6ê!òC?ÉèŽÛ`Ë?¸'ÙI†&?¶TVÏõ•&?ͯ7²ìl?ÉNÞ<òá?Û@‰ïÙ?ǯÙÍ|[?ÂVk!61?»" f…x®?Û¼´À€R?Äe¬•}]×?â·Nµ½?²_L¢¸)¼?À¹[Øæ-?¦&iiX¼¸?ÒCv!of?¯?ìêy…þ?Úõ,¾ò;?°R¸
ùf?ҙ2;;•W?°*ýË"F?Òqµ˜xn?®ÆÃR¸z?àÜÒ\?Æ–Þºq<?Ê]Eˑ8w?ÁÝæk•‹~?ѳ[`'«®?Å~'<¹?ÃJ2¼skæ?Á
üVìå‹?Òlç"Ó-?ÈÊ	ùÓëû?â¼ÝQ»p?Çäqf+Þ?ÚN¦Ö÷?²ÇR®[o(?È\)™Mç?®ÄÚ
C?كLJ?³C¾k)&'?Á"6³Æ@—?¦Xå˜we?×®óEåðé?ÛBö?߇q`6îÌ?ÁqÃ*¦aMIXED4FGL J1203.9-6242¿ã
ôu濛¿Õ£òfa´À7럓®žÀ:ƒÝ ×æÜ@åÈøן@lû@}ž'?«uPºÃú?Õå@Ìxé÷@(0ítA@ÁÊqRӍ?îc'ŸÐ¿Õ†šË'¿áW›ÝÁ'°¿æHiü¿ìòFñ'¿ïÿúVrÓ\UNASNone3FGL J1203.9-6243?a¨7ßòÆÀ?_Y—MÊpJ?îÝ:œoH?¡ _²bÖ?¡Ò·Þ®@? ‹ð}oÜ ?'x0A'ô?Œq¦ 
2?çõ•[
Š?º¸þàV}¡?Ï(Þ4m	?ºUÜÞñE0?q
«±–ˆ?ŒqY&Õ?ìÕj­¥j?¦ë¥»G¦?µ¦‰^ÔoÛ?¤çՅ»½Ç?r±ë`eåE?]­›Þü2?ãLÁ­Æ?©nÝZ¼ú?Ù´ö[*b?©Jz¸Ýöy?fÒDŸ°ú?blM&=@?în=ußÞ«?¥[Èãë¸?§»;{'XÄ?¤'Zz¾ÅË?w/4a`·?€ü7LÉ?è¹QàóÊ?Á"vݒ?Ìa>Ýž?Á	.»1øS?|Ÿd‰Âa?}2¡…ÓÁl?íª'£xb	?¢··Ù	˜?°á|›iÏé?¡»Lyƒ¹-?Iuvß»S?9#ÑÊ3˜?äüß*-·?¬É…݉_?ÖkˆŒÝ°?¬ÄiÐý&PSR4FGL J1204.3-6111¿Ù'©ŠtÛ?ò¬š'^ÛÀ9Ù¨g'¶QÀ;(Ag©]@úhýoî@悀x`?ԐY—Œy?àœ<ÁÒGá@
ƒn´é?þÀøãÖÿ?ß{ûú?ƒ`MŒiŸ¿çÒ(ÁÀ)P¿í[ˆêዿè.]@L÷*¿ïÿÖDDÓoUNASNone?¸KúÚp1=?À#$I'ÍG?څœº¾àÙ?Ý3¡}=ÃZ?ßgdÉ+Ø?ٌG"?ÈÆð#üs?Å`6‰Ýl‹?·ø2¬'ª?³oMî.ù?æÏ=¡ºê?Äô‡³µq?Ó¡":?u?²qéôN<?Á©ÎLŸ?¬ß@•7w?áÅ1JOÚ^?´®/àÄ¦?¿G›*½™?•z‡@â¯s?ÆÑΐ¦"?¢'²È(k?æb˜ø>¬?£N€Ø·Ï€?·í½<#Š?µsî)âÔ*?Ä5¼Ä?ÌBDUõé?çõoPÉ?ËálŒEH4?²'Ž¦{ž?¸9ðcý¾?ÀIq&ù?¼ì=Å!K™?驉¥«~?ÁÂ&փ"Ú?ÅΛ"Èæ?¨ä e&$¡?Â{öñc…?°»^*K¼?åí[^å,"?³q*Îîb?ŸDóݯ^'?6ý%ÖÅ?Èð¿4!´?¬Ö/ù¢+?éÜ1)ÿ¿?«ö;š°¦ïOTHER4FGL J1204.5-5032?ïó±'eí½@'Eík¨Å‡À:]4=õ.À<ˆ໗@æKùӖ@œ…Ý$3?Æ4¸Œ£è?èΙ«7@ Ù#¯2@cLÝ(d£?ïìQ'(¹³¿Ô–)ÂÇt¿ÉôuˆBYA¿è_[5z`¿ïùΝ²X¿ïí¦–Ø:UNASNone?ÂåAûD{Ò?½Ñ6ÞkJ?è(i+ÎÌ?ĶŸ"–¨?¸ò2¬¸uÌ?µ.ŠÝû?²mQ+à'L?´mN\æR2?é«(K½\†?ÀFۂXp–?À¶;ˆ8Á?¹K¦Yä?Ҕ˸"u\?²i8‹Ù¥?âS®ž—
?³´e 5í‡?Á‡®záH?§L¿"¡?Ò»'|á†?§¢¸bmĐ?㉈8Œþ?ª6Éš&?¸ÅuÍÆù¢?š¦rp	þ1?³ÍM:ƒQ?®?ß°Ò9?ê*—MŽ­?¿‹>.†G¥?ºÝø"âáÈ?¶^‰yƒ'&?£™MÀ
‡ä?­"	fúï?ꮚïÒWÉ?ÁՍ¡ÏÚ?À_@Ï ^&?½;;C¼²?äߺó?­c8s3àJ?æø²Ù(K?²aú¹«W?ÀxU€~Ú??§¥…yëÃ!?¸V†[!¯j?›Œþ nïÔ?é—7áæ?ªHúR"Œ?¿d¿æ=å?£è(å$ÓPSR4FGL J1205.1-5951¿ÐJ¼O.Äí@ü¢¢&0À:1š‰ƒ¡áÀ;œz'
‹@°†ðõv@…õ'^éš?Ç7ªÉlÆ?ª3¤r:¯ÿ?漺Ñ!Æ#@‹9&A³¿âîO~mnB?ïøYþyC¿èˆV{6Ø¿â­RH¢0A¿í/†ÖHv'?Òja}ss?UNASNone?ÕêW®Î?¾)Læ&?ƒL½k?x¥,õ¬j?äÄÈl­í?Âöî`õÂ?äþƤ6"?ÇZ.¦æ³?'þ¦$²?"ŠgÔMë2?Ô҈V-ç¢?ƙû½ÝÞ?ãQóV"#?³"º6&•‡?¢˜îϱ!®?'ÉS¤?צ>>eQ¥?²¢Žm"Î?ê¬D¡Å?—¯ÎJŒ|a?–/fâò"ì?vðPš­+ü?‰œTY?•Ð@mm?ÌgL¹?ÀA&öRÇ?•âe˜é£ü?'loK·Ú?èIRï2Ÿ²?Àýû)<Ët?ÛƪŒŽ¡Ì?ÈQ •¦Ø?£beÈ(?²K*'Hô?àë©Ó'R—?È(Ñ삆?ÔૐUçØ?´hµ9÷â>?ª›£úw?•â·+,À?ãåø†¨¿ì?´Ô%Õ;V#?ãrŽñS?©á9CØä?¨"«ø,?'ˆV#˜Î}?Õjg¹?¨£(mð9MIXED4FGL J1206.8-6038c¿âF`‰O
?ü4xã@¬˜À9ÌAƆbÀ;%ÿÜđ•@Êæ¼7(`@.ùèŽÊ?ÐÒíÌw?Ï`Š™ÌoZ@¹5v'\@qæOx?ì¿-b
翱ɫ/C9'¿èöĝSb~¿ä¶‡æ鯿ð?ﶞaUNASNone ?êpA98äV?»ù)C'žJ?–·T?"³{ÚüAX?ÃhPcDÉ?º~l0n¡?Ö©åtÁüm?Ìðî<æ÷?³\zŠåÀœ?°¹IâG'?â?}ôf?̯ÃÙß?à]0IAp?²"^¦!¿?³e.¬ùŽ?éí¥ýƒŽ?Úl\Ô02<?±"N ˜?ÕåeŸìïØ?«^¹lõV?¼Êšnù?šé9§†L?át"?¬V'{û¿x?à¬["¾R?ņ—U¾ð¹?³Ll]Sö«?«qrR¾Ð?ÙÔà1ƒ…±?Ō'Ï>ÛÍ?ÂîÞBs "?ÀòÃÈRzÝ?ÀÙEêM™Ä?ÁEEMÖ¼?ç
öôFA?ljÏJ?r?Ñe}ÙÛº7?¯`_K¡w?Àf|ÿ¸?¦Þž.ÊZç?ã3¡Ó­oB?±´9?·ÔS—SYž?šùâ~?ĝþ}
?­‰t3]Äd?çÞ1Íò*™?¯è±õOÇMIXED4FGL J1206.8-5836¿ÐiÈCƒÀó@…`&±EÀ:»™ž¢À;ØA'è|V@ê×yÎù@I¥ë·sŸ?ÕÙ*ÞÐÛO?é›ü_âhÀ@¥º9LR@YCNa?ïôáÙú2¿ß1É~X¿å~®@ð‹¿ï!ÃÔֆŠ¿Õ=ŠÅ@fx¿ïþÿðÇôUNASNone	?åwp˜¤a?Çr#50°Ä?£&Ø6+mé?¡Æ ·	àâ?Ò¬CÇÍV?ÆT2´T¨E?âÝ®ì^"è?Ç.¡Håw?­]ave؏?¬Sj¥Ú'{?֘õøȱ¾?Ä.–²DÇk?ç扩Xö´?°^=•:?´ïӝ€?¡"½»ÝG?ÅîPqÖr?ª&… ¡ò??ç…²BC-?¦³Hp ë·?®ÇÇ9s°?—½T抃¿?ÌC÷wV‰á?¢é[ᘯæ?áQ×ä'?ÈÁÿ«éŸ¹?®CWÞZ¶?©>·%»?ٓî,v‰'?Ǻð"Øê?Òó¼àÆ~Õ?É宛…?Â-p¨«ý—?Â{]èØ4ú?áúÅdèPÑ?É[%†ˆ€ÿ?ã2oéÇÚJ?³Ä£ÑŠ!?À›Û=Rò?©&J½\z?їÒ?䂲?²—:ˆ€Ü?Ö½ÕÆÝc?²h¨ àš;?ÁÍÅ	"Ø?±ŸDiÁƒ¦?àYbZH˜?³Š'ð¬¾MIXED4FGL J1207.4-1840?큮¶Ó;@E}NÂò®À;@Ë]a'À<˜Šï²ªã@'¢ivç?þ¦êjl…d?ÓÒÆáÑ@Ð?ВôÏJU?ýkؖ.«@(*…È¿ïüþX`f?ïü1©Æ7‡¿ÙÓåŐ¿æ{°&äp¿ÙÿÛíÒ¿ïÿõEq#UNASNone?ïÛjùr·?dl‡ÙÚ?Jwû¸V¼G?@3e`ËZ?m÷'0?bpѓïô?ïԵрD?rw…Áæ?HìûÓF‡?S7†ˆÂ?r¤™ ý…?m­‡å?ïI@€?"þ "?nŽ¼ªÌ?p%‰hÕD«?"&K(é?'Í´'â'?ïw'(Z^"?j[hj?eh9}aÄ?Nlzۀ}?ŒÜ'ŠgàU?h~>jc?ï·g©†¢?u`
u"Â?V^C·wÁ|?L!H$ò?~´èºŸØ?s›®šNI¶?ïo±+½.?W:ñ\h?_$lԑ?i秷'^?ÈãÝå?ŠK·Ì?îÇ=ê§v?gÎÂÝ?z¼µ®õ5?y%zÂo? Kwéï¾?ŒP3îڊ?î´¹||Â?‡›{ü?pú·¡®oK?e	e§>–?¢•G·N?†"ÿ&ãaAGN4FGL J1207.4-4536?í͂ù*_
@0"süPHÀ:tŽ·¾GÏÀ<}MPëªÞ@`Tßd?ÿ<¼æ¥¼?Æt~A¤e%?á7^3'þ@#¥ ¶Xí?ñš0Å´Ö?ïÛi³"Ü¿Úï
Kšˆ¿ÎÊ.·Îbú¿æŒ x°ì¿ïÿ
A1"¸?ÊĦ}ìUNASNone3FGL J1207.6-4537?Ùs<D¡<?Æxu›Qn?ܧÐ6—If?ÉàžèÛB©?ÃÉç	Žôû?¹LzٚM?Àá£Q0ý¬?Á›
Ž_ï?è­ómË`?Ŷ€°®‰?½WIÂ/©«?¶;l"R?Í|‡(fü?¯	[Ü:?âÓHî?³ȊB?Ç7Hõ™L?ªÍÄëî*_?Ó^º)JëÐ?§ÇÈH\#è?àíÿý¦´_?­¢Ú^d?Ŋ‹´©•e?Ÿ.Nèˆy"?˜%k…›F?Àn¸¸v\0?âkú{Á?ʞ"!¬ð[?ʳð¨Aµ?ÁuæóáÜ?¬°%÷ù:?µ¸Ý¶ç«?êÒ$Ç×è?Ä<xлÂ?½)\ED$?¼œ1öŒ^?À¹1q^‰p?§JhFú?åóÚ>‹'?³¢îŸ èÅ?Çx‹%§HH?®<xÇù?À+œn"º? V€þã¸[?ä50H·d?²äº¿½?Ï)CBŽµ?­z8?‡PSR4FGL J1207.9-6443c¿ï¬ÍKDCÀþ}~°àÀ9ÃÚ#Íd¢À;@+ôzÀ@ü¦¬| @ÍG`ç¡d?ǎ¾^9ò?Û`–ƒ9°Ñ@"yJ@«"6‹­H?ï#BÅwmö¿Ý}M¾NÚ¯¿á~@Ï~¿åOãm"BJ¿ïÿþÞ÷?íkP`j£ãUNASNone$?ÃGLg./?µ"ºTب?ÂuÙQ{®Þ?»¸ËŸ6wÇ?æw؇H½?Á•êÒ50R?ÛyMÑ;"Ì?ǚìы3¶?¨×öfB7?¦VÜXÂ?àµÙ±Ñ?ÆFyÐÀ;3?ÔÀXíyb?±2U™ÝQ?È´€x"î?«M
'¶?ÞåfÕ)Æ+?²ú¼²îíC?֔€‡œ8}?¯Jœ9!E?¶ Æ®†s?"ÀÌâ'ó?áá¦æ*¹4?°=적ß!?¯Ô›j'"j?¦1õò:8™?Ã<õÎ<¨A?¾^²l=.Î?é3xÕÿ¦i?À±Øú~P?Á'¼®,ßÃ?»]}èÜ?±ë×ìõèù?±ønʺ®$?éx•ÖŸ0?À"<¯Ö?ÃSZö?§ý[Ê{ð¯?È¡¾&ýÖì?°ÎzŠ=cÁ?å¹ï¶—è?³ïÎ{'ë?»é|A*Rö?¡PÇ"%à3?À~©©?¦œ ¿_žC?è{ˆõ»7?¯«tÆ"$OTHER4FGL J1208.0-6900¿êŒ"+ëmÀÖ¢?ZˆãÀ9ú¦wÎm·À<åaïa@*AþR*ð@âÛ,!?À9­å×?×ù%ò-/@ÅJ]ò#ž?ü«?#VqQ¿í¯/˜sÿ¬?ßÑ%ʟ¿à¬ÅZèƒâ¿å'¹ñ·é¿ïÿí¡Ā?é7"^6UNASNone3FGL J1208.0-6901?É¿X=Œ[?ºš)%W?Ú8…ñ#ÌÁ?Çõh3_?ØçêaªŒS?ÃàµH2?Ï1z-Ï?Ç¿½3–t:?ÔH¬‰,ÜN?Å"O¼'ýT?Ü/º¹‹Ê?ş°CÕ?Ν´	Ì n?°í™Eí½?àWI°3u?µ	|™mI»?Ðg¹ˆÞ?°ŽÔˆqÃ?âÜZñŠ"º?­õ䦼?ËRR¡?§?Ü{ûÕÍ?ÉAçV?¢Ýîó"5&?µ¢Drê'?¨›_­¿µ?ÜÒxà¯?Éõ-éó#?ÝÄöa6?ÇO-/
3Å?ºG"۾π?¾¦¹Ÿ•Ô`?Úe*'¶â'?̐ÏÊÇÓ®?ßô6Yi?ÌlJG6¼?¿rMqÅ6£?¦Ì-eu?ãêb;?¸x•>(?ј|Ê<5?´¾Cõ¿f?Ó
þž<R?¯*¹4ǝ?ÖöÙ*K?µsoeŠë£?Õüëü›z"?±Ö­of«MIXED4FGL J1208.2+1158¿ïó%§Œÿá@QñŠ '§À;<n—OßÀ<·;÷ýÒÿ@¡è:@g¸Õ¥¹?л›nÛÖ?ÃsÞt$?óèÚI@E¹F]1‰?³õ¯o烿Þà#`"*¿æîÉp!¿Ó(ËÑ$J¿ïÿÿ" 5•?ïÿú@ùDzUNASNone?ïvôçPº5?"YqF΢?k
Y¼Ø5¨?oð°ºo?‹o¸#çI?'¼Q"´?ï›T%µàç?…¿T¶ˆ	F?_§ƒï8´‰?dÍJ'Ÿ¦5?…6#§?'#œÛÏ?î´ßëJç?–.K¯æ>?ƒxjõ?†&%\¬0?Ÿáœ'g©?'ë6켆x?ø1C^?j@L§²?f~§I¶P?P®à4®c?"Û"I,Îþ?fö®ð³§?î΋÷§q?ª"hRØG³?zýóu¬ú$?‰ñAúGñ?ŸoFkO?¥übØ
šB?ïóÅÆ.‰?Q†oC?iÛV	òQ'?x½³í"UÕ?™Æ†'ß³?šöÔÞF.?íÑù3Ýþ?žÖ@Œ¹Â?ˆ7¨Siá%?ˆ¨s‹ñn?¬áÖWÀÙ?œaÑ3íJú?®ý?B?SË5`q?=Ã%a¶?q\yµd?£^§á¶?Š¤*і´XAGN4FGL J1208.5-5512?¶¯'«ù@­\œ¹À:Š÷mŠGÀ<'8Yã¡%@×XìÖ-@¥Ò! c¸?О#y+æ?Ö½±[­$ç@P—\¨wƒ?þýîþOü˜?îç%pÔ)¿ßg"ÄËL¿åìÏ¡"c¿ÞB(.rý¿îõõO¢Õ'¿ï#'ŸÐ€UNASNone?å9›Æß;Ô?¿òMür?¨_È!Z?"¬'8?Ó²Bu£ù¢?½©9†Uç?ámÒQ#¼¦?§'{÷à?±%é0¡,?¥¦H7SÍ?ØâÑãÚQè?ÁOà_s%?êc>ш?§ÌAÇ*	?§ ÄãÍ®ð?"Ö·+¬ª?À©š`Çs¥?£½:juƒ?èmF/9T?–fúþü"?³!ú\Å+W?¤VnÉ!Í?ĺոr'‡?'¶†&"ªó?Ü=vÜ2ùÛ?À|ZÄ	?§óÒÓª•?—³­^Jø?àbd«ÙÁ?ÀdVîƔ?м™D›L?Àƒ)`Kš?»¦'˜D?·á‰a©?ä-0a"?ÁåI¿Ö^
?åVkA
?²9¦ùÃ>È?±ë"6ì	Û?œB°r±ÊÔ?ÐÙZË}—?°_d4?ášNuXó?¥k&¨V
?ÀL¬:ù"?¢½µ†áž?Õ²uFÑY?¥
9Ǟ{MIXED4FGL J1209.2-7635?Ù:Vn‡Ù9À+×ÆÚD""À:Ûe¿wy´À<1"óg°@5°!›[;@›Y<²7ö?˚¸Å-ò?­&û#9t?㑺ýíV/@C%<û^?ì³vð!e«¿ÂdŽŠqÞj¿à&}­ªÈ–¿äÜ`ô6ž"¿×€´ÿÄ¿ïθʷH×UNASNone?ï9/Zæw?ŠÂb§?Sí7dfû?G>CVÉ¿Â?—›ACÕ}?‰þÌ_zË	?]ö!Ò?Œš<Æs±?beµ
<›?ii•{©!?‰¾»C
âI?Š%éί2Û?îè•sÖL¹?Žñb³8L?uß¹ÛxÍ?t;OuTß	?ucû®'?‹¶¬ð{?·øÕ>?}3äÃ-N?p%$^Òpí?TÚ(¢¯ñ‹?¥Â?ö¨!ù?{×Êoåí
?îPzZ¨ÜÇ?›VµM½¿?h$b«n²?^'Ò'Jü?©v4c‹ ?š"àoØ?î¾Âᦖ?§d¡k$Z5?r	K$¸éb?€EˆÉ0kÉ?¡Ò¨`!ê?¦j¸'Ãr?ípÔhnö¥? Äږ?š?‡~P
'¦?wŽ«vµB?±‰'º,"?ž¥×PÅ{†?ëŗ>J"w?˜bYý§?ƒ¢à•ÚÞ?r¥¢1‡ÓD?¿^éý+±¬?—sp
ûAGN4FGL J1209.4-6421c¿ïù™ƒ–šX¿ý"€Û\²ˆÀ9"$¼wêóÀ:÷bLLà@ÏrÅz%@#_=}9?ѱœÃ,?Æì¿o?ÿˆÑ•‰i¡?þ\3!•{þ¿ïJAl±Ú?ïõºAYç}¿äÔ6þÄÁ'¿ëôÿñ½G¿éÁ2?B`"¿Ùúc
UNASNone8?Îg¬?A<?Æ&þm?Ý?™c,}¿üã?•åp…óe?çšû‹üøå?ƌ§¥˜Là?×÷É]š‡?ÆD{x¹>?¤€ŒJ";A?¡ðiIš¨¸?⼺í§8?ÅM¸«¾Æ?ÖÝ+z"U?³­Ýlƒì?²«4Yu}‹?žæ|З$?â<	ß/ƒ"?³Ñû†òÚ?Õú¸'èÓ?¦/Råˆ?±ÖõþFò?'q«á<<ê?âÇÄþÞS?¦Š;$:¿?»>Í<«¤V?¶4cäõÆ? |®Í‹Ñ?Ÿ¡®b"ÏÏ?ë[kÐLx?¹©¦dÙ?ÀËæNdMC?¸†Ö¯åH?©Ð_m<³(?«2A5sb?ê0u"!}?»ÃE ¯I?Ç7b«#V?©`7­~Cv?¸ìf«f½Ó?£Îr<©È?çš®È?®ù¸úC8Ë?Á·Ø"+E©? bÏ°'^¶?´SUK7Á? ªØÖ!]"?éŸ1Å02?¦;ž·q¹OTHER4FGL J1210.1+3241¿ì³ç^ڒ@SÞ\å´$_À;ÅÚ(ÕâÀ<é(kYn@!\tWë¤S?ûYê¦Òg?Ù>4ƒ•KV?¯ô¾®Q¶?Þý-<ÏN?ýíôOG»Ö¿ïþh›Œ¹?ïúµÞs¾>¿â¿Àʶ¿ïsøö ƒ?î0?)á{¿ïÿ¸GʐUNASNone?ï‡Ô9 4?ªvQ(J?P†¹'‹ì?o\Ÿ?¯C(?‹úm&…?¨ðþO8½Û?ï™Ùøs3?"€ÔþSëU?`Ú7x $ô?u¨n¯R«?…‡û"]
4?hmnñ¹ç?î]l¿hW¥?—‰~±#¡?'¨ðOù‡?"Åÿ¬‡­À?¥-	\üÙ?•©°ô‰?ïŸzíîÙ?v&L
i?2åNXo`õ?3ËÐá^ç?‡Š>ý7?v²ãX³­?ïmbtqõn?¡[@*=«?X?Ž÷Ƹ?dÙTè¯?Ï¸™Ìà½? eS¬O~Ã?ï͆¯?¬Àé–fq??gKR0Eå?€Y—šÁ¯ß?›ÜõüÖ\?«2®TÆê?íIÑ>eZ<? xG\Wf?Š"¤&ݲ?Œl¼™J€?²^åؾEì?žJG$kj?î›|ñ0s?™'4Ð$q?EÃ6Éß=X?UBË`Iï?¥ñ3œš?™vÒf·šAGN4FGL J1210.4-6250¿ïv·FJ3¢¿ÕmÒÁXzjÀ9XsHÍÀ:še"¯O@¦—Ìdòô@ø¶zzða?Ð"Ág	?ëøìæGÈ@s@ªÀ3?ùU®ˆ>(¿ê w~瑟?¼ÚÇ·9<¸¿ÜK¹ý<VH¿îz̺XV¿àŸÑß[E¿ïÿ2Ȫ(UNASNone?·îLpP]?µYÚrïå?ºL[ÁOs¹?¹ÔQõ{?鸪ù¾Gy?Á}¹ù$]q?²ŠøB'?µiÁ¸z8?Æŗ]n	?ÀZÌC(ãh?èHån{«?¾ôi°;ƒ?Ã쳿à€?ª[Ù<N?È
ˆÿt¨?­ü f@À~?åV"Nj¶?²Ê0XØ÷7?µ>E?s^®â:¸?ÑƂ€x`d?±zÅCS¥?æ—ͨ¦
?±WQ÷.?«kT]ÝT?¯CÞ°‡ÄE?¾6m‡9g!?½4ž`[h?ê'}L0–?ÁY4U-j-?™ì‹WWB?¡Â'h Eˆ?ʲþ—¶H?ÄÕÓ*MË)?èŠ@ø1™D?ÃñXÊhæÁ?½*R×ñ̔?¥È
¤]?Ç°Ÿû2Ì?±Rlò78¨?æn¦5";?´ÏՄ›?hY|k˜?U€ÊÏÌM?Ö%ß2ç?¾F"ðPpÂ?äÕ"Ù¯<?¾48¬Cë<OTHER4FGL J1210.4-6100c¿ì™Ïª«Bl?÷|…Ý$2åÀ:@ù¬(èWÀ;igI»4õ@ H.}ÁÌ¿@‡åÝ?
Ø?˪µJÐë?²ór}öÑ?íá8ÿûÎB@VÃÉBÿ"¿ëü'§:?ác¢1пÚ*{žÜÏy¿å¬vJßø#¿èÁ‹ ²'¿åWÃ Ô ~UNASNone8?Ûø—Ñmpq?Ç
IÔy-W?|äÔ´Wu?¦¼,ñ™˜"?áÉêm­¾¦?Ç"(ÉÎ?ßúœúÞ>J?Ï&ꉏúù? 6¶ˆX?˜" %	Zå?ßáHe±?ÎvÏGxÌ?åìÝÌ#""?±æCÏwFê?%) ±g¡?'Vg¨¡B‡?ÒSñÍ?ìÞ?°ëI»Ð?è¿Ö­~Ü]?žDuš®Š?'í¿nfü>?fŒ‡ÊӐ?ËÑÉQÔDL?ÚðÉn¥?ÌzWe}Äb?À…[@ß?Š.%÷?"Ÿc‰Ç|q?èx±4?À³\ÐÝÊî?ה©%¹ß?Ê*¡Ý=ã?•"et›TÒ?§•FÌÏ?ã‰AÂíü?ÉÀCËö|ã?چpGÞð?·ê™Õ«M?«^Q¢?Ÿ)µÕû¥?áçÒÙù}?¶­v¸—-?à ½µW»(?­CçàtU…?'H—÷•?€6#Ö.'m?ݤ°'w¦?­5ÅYœñ–MIXED4FGL J1210.7-6005c¿êÆfäx@	1*À:n+ë†ÌÀ;k*þ±K@ 	ÃÑ%¡û@të<#œ½?Õ[H{úù?ÆLCe'Š?÷&q3I¨@$lÆÒ¸¿ïøcß"Í?ïÿvmD¦ù¿çQÁÚM¿æÂ:½k/ú¿áFmlêäæ¿çp$ sRˆUNASNone8?ê'
™¶õË?¸®FNé"??šG[´?zB©¦^N?ħÛóþŒZ?¸"""ÙÇ?àãù¹ŒJž?Ì_A⁩?¢ñþ¾ðâ?­Óüq3?ÛÙ̵$åh?ʃåõŠ'®?å¹»OCVŽ?°ÊN Ø`?¢âŽc²6[?–"ëˆ8n?Ò07•Ãv7?¯I.#'B&?çº+V^Ë+?¤·2RTäó?ŒÏ†li€d?tð'ù'?ÏJZA?Š?¤œ«fJ¸?âÙ£9a?Ã	¶Hb*©?šqŒø,"?"}î³ãƒ?Ø¥©¼kD‹?ÃD­%‰õ?Õ>
áŸ0¡?ÇWv¼þV:?±"'l,?¾#݈dp¡?ã>v=š?Ç`«³À?Úö
þáœé?²LÊ?!?´XQŒbïü?¢õA~?ßóàž!#ø?²/pq"«?Û©"Ö
…Œ?±¨d/<t?šæ÷_6`(?ã±¸÷Ü?áTÚEÂh?²\FJ8É¥MIXED4FGL J1213.1-5957¿î•@…šøÙ@ø¨ó©°À:Ç"hà"À;²þ¾·`T@Wÿ¡`bk@ށËFºÏ?Հ"ûOA1?ãÇkcü(Û@F{åS¬?üü‰Ñ$ H¿ï÷fÁ1
?ïúõ—k¿á£8I©"¿ä\«!Vfê¿ïþæŜVã¿ßëXZ4)UNASNone?ͧt86'Y?»ÏI:ãX?ÔÀ›ñ¸"‡?Âöb̗·†?Ük©ò,WÍ?Å^Å	Uw?Èòœ÷¶Ê?Âÿé ©>Ž?Љw7™õ?Âø
£˂?áÁ;¯µ²?Ž͚@ø2?Ö¦ò€™ +?±I™†aI?Î1^ÁEHù?°)~½­ò'?Ú@^Ä;Y?±Åj4<¢½?сmG	°?¢g´µ£?Ó#<L®Ñ²?¥»Åo^¨D?Û[VmJ]?¦´ì>:?ÃÅ
Fç?´ÕœvÝq?ր-jyùõ?Ä5ÊX9Ž'?ßõðb'‹?Å-¢>r›?²"CiBV?´Ç&Ž—Úh?×ÅÙ­I¾?ÊZ¤þQª?â$¦oÞ?Éß߮Ѻ?É9\9‰0?«™ò_ým^?ÔL3»ªvÈ?·''Õƒi?ß(£Ññ?µ³'†X]à?·D¼"è§@?"'Héê-?ÖÁœöxö??±ðÛx-Ú?ᶙò&où?±Ôšæ9Ÿ"OTHER4FGL J1213.9-4416?ê·¿T>E¶@2b€'،À9ÿ'xë¤(À;÷%=§*|@c®%AÙ@[¹™ê!q?¼b?PÍÎ?ÍhŽŸ? Õ@m.¼«íY@aBŽ?ï»|þX`?ğÚ{aU¿åZ³uòW¿ãû}å3 ¿ëmª]6;ü¿îlЮÝ*UNASNone3FGL J1213.9-4412?âÉßü_j?Áyå'I ä?Òùï2…ìÇ?Àwß_¡{:?½ÉJ¦Q'?±"Ôô{¡é?ág¾øp6?É#¸õ]f?Õåi{Ĝ?ƣٌVm©?¿-,bMkÝ?µ8}!£D¼?å›±LNô?±QyÖ/?ƾ†MÚ?«fëQµ8ã?ÂÓ{€ê ?¦UÃÒî?âÿ\ÍÑ?¡õw?@v'?ιæ²hT? äéÏí·?ÅH©
¿h?–¾ÆKi»?ӑ²_ŠL?Ày>m›[?árюl?ÃYåÜ=?ÂÞӟú±·?±¤´ÊøaP?ÔvÉõE֓?ÇY[_LA?à‡×ÙV",?ɾ!£¾¶Š?Äó°B)?ºñ3g=?ޗMÇNß?¶t'à$àŽ?Ó~Œr"?µ1<´4|>?ËÔM	H(8?­»½ÂÚ	ë?ÓZôB\œ?¥sw'(Êá?ۇeúÛ©?®é‡?:W´?ÑY¥ÂÇ»?¤ÙÖÖ¨þMIXED4FGL J1214.5-2318¿ï·Žì0Y(@Cc‰!S7À:ӕÄ"`À<o]2K­@\Ž´
c@?ýהÁÄO?Ô(ªÄbC?Ñ.…dˆñ?ÿÏ'T·@øSK+¢p¿ÕC	ËÜ?ê#X)ŒÁD¿Ó¬¡«¶Ó¿ÞӎóMj¿äøSδ-š¿ïÿ7¸Óñ"UNASNone3FGL J1214.4-2315?ï俖>¬t?YØ@3!ñ'?CLtn…"?4÷ÅU™ÜÆ?fÖ¤çÖi?V³‡¹?ïÒÞ}àg?rÕ½èR—+?LB
¢$›?SÙ^øÖ7|?sgÏz¯§+?nKñ𛧝?ïz©5æ8?{Exfbˆ?gC_À¡?p%Ák&âë?†P½Ý-´?u"
¤ØA?ïª\ñƒÍ?rI$÷9?s<R"?S&µ¢?˜†Ô_žq?p¿"Sx\?ïÅ;µ|'ç?onî#q
?T)Šª Ít?H`¬jrh?xW•®€ñ?lË_øØ«?ïx4À¸'µ?Šˆ&äø?^ꥩ‰?e†ô䋊Ù?Ž{$TY?‡YW§_??ï4A°Ïk8?‡žbÄ)ìâ?r™ÑRž@?w°ØÔ-Æ?"ÑU˜nép?ƒ"ĨD?íëo³Ùh?Œ;óigà?|á¨þ?iXdŠÊ?­·¬:Ä?‹oD¸TAGN4FGL J1214.7-5858¿ï
Š¯Æו@'Ä$#À9¦`;©ú:À;kT/,=v@ÛÌ{O,@-¦¿
"?ÈïcЉð¯?ÁÏ+KÞ$ä?þ<xVRòì@•€ZXf?ËM¹Ü°¹¿½håq´MO¿é^´ás¢å¿æ1neZοïÿs³VB?ï¾h…ûW$UNASNone?ãïÜ̺?ÀÛ}ó(‰À?³Wd"u?ˆRV9¬3?×ø³¼?À¶nØaÍ?ãŨÞ'Š€?Ɔ^ߎš?«)I`­P?§U:†C
Œ?Õ…›@ý?ď`E²?äÐ$óG?±æ֟o®?¥æ#']ŠA?"W&kÝ?Ó¢óa®h*?°Y'üôG?æ%f¯›À?§\w#r×Ö?ª>ÜÁúp?ˆëá37ð?Ðmpfs?¥6€_TÜù?×ý¹¶"D?Â='µˆ?¥ÙâgœO	?¡¡*mÍôü?â£Þ|«)í?Âþñ(2	y?Ր°få'?ÉéS"ü?ºâíS2µ'?½Cæ¸õï?âYýï¦ä?ɗ•h1—¨?ØØÆTk?³#%ÊW1?³YííÒ؊?ŸÎOZ'4?á(¶¹Ô¼I?³¥nâ¿Zý?×û
h¿?°eÑ:Ž©ù?¹…¹ ág? ‡2Õ8'Þ?àÑ×;÷¹?°…[՘í/MIXED4FGL J1216.2+0537¿ìeC'­Å@P»>-b9À;}JØkf€À<¶]ŠÒS@ R"²,?ÿ«cÆxö?ÕV¶JªH?Σ€ùÊ?êžwïû¥þ@	&'=TŸ??¯®Ï¶·Å?¨Ã=ë¨¿ÔÝç®Ðc¿åÕuþ3÷ÿ¿Ü4ÄØ·'¿ìÐ=ÊeêUNASNone?ïèvÄÇ?Z3Žt
â‡?Bcs¬ö?6ßð5O|y?cI"ÃQ?V§ msJû?ïÁÔ#-W?zÁ Ý?Nr'«ZíW?V}\"—?{iCœ*—?wjÔæÇ?ïjüC Ö?"¾'
M*?fx´͍`?iø·Zg?á"ÉÅ;?ƒ g;¿óò?ï†Çs¶Ií?lBÕP*?X¹Ä•j?@ž—ÍÆc?‹KkÊd£Õ?l
c0¢µ?ïÅ Œì¦Ì?rMÏ\BLá?S±Ê¶ô¨œ?Jkuø(‹'?xCFü;ÃÜ?plKîñð?ïS7™¯x?˜^µ­J?^%+gõ£)?ibè¸|¼÷?"¶º. º?–"•6Ğf?îòô(ÜB6?Ô§¢|ß?r°—5³åy?tA·R¦§?œõUmèâ?qC5Ë6?îœ)!?Œ¿†Ã'?h%1:|'?[Æî§0?¦ƒì="Nö?Œá¯R«ƒAGN4FGL J1216.2-0600¿ËÈ-ß>òã@Kå2µ^ñþÀ9ÈÏuôxãÀ<,νgÔû@¸™nÑnó@—¯ê=öÜ?¸óÓÌÆAÃ?½Té;mie?þ±Á
{é…@D,²™Æ¿àsûz_B¿âž.>VÒ˿蟦=ìʙ¿âtŒ>'6ú¿ï¿¸Så¿ðUNASNone3FGL J1216.6-0557?ïztIlÊG?'(¿5Yã?zÏEK?sÑê\ltî?"Y%33ê®?wËÊډlÞ?í÷VÄQ?²
nxÒ¦`?³Ó¢A~?¨×~½?¡°´òž?1?Ÿ¾5ãÅ??íö-ñLUf?œ	OÚ¿ÆØ?ŸO3ÿ<ßÐ?•CAۂø? õ†êÀRÁ?I+ø>[)?íupG:Ò?p»BÐy?¨*?ã}ä?‰kù[Ǒ? ~»ª:?z5Œ½´Ê+?²Ÿi?™5d
́?—I–\SÍ?8ðÒߍ#?˜Ø%(U?Žxbœ•?ë7‰f›•r?ÁwËû¡÷?°…ñY³?¸HŚìd?¶B.Ù\R;?±çÕtK?ì4p¹6Ô?¤ÚK6ErŒ?­éQÍ.?Ÿ¶Eæ?¯šő
?—W-'DV`?éGƒb(G?©etAþúˆ?ÀáÂûñ07?¦¤æ8_–?´µð{ùW?"£¬NköAGN4FGL J1216.2-1550¿²TBô«7@G5ü;OaÀ;W%­AíÀ<šÖvš@ JB¾@
¤‡3f?Оi¢…üY?®®£Áæ"Ê?߸©)Y•ž?÷¼"*F¦?æáJ2S9¿ÕãvÇÝyÿԒ/BêÊ¿çÚ\FQô?—˜×…k¿ïðÃhŸýUNASNone?ïLȼœÔ?"¡†Ù뜰?^àXãn½?jŒ-"â~?"'aZƜ?‹úÎG35Ü?ïFb,šè¤?"‰Ò M?s*৕ȹ?vÖì'è3?'iIœ±E?›©"ÂI?îö¯cS?Œ6cåDŸ?u›<ᤢ?uE"Zÿ£¹?›åø)ãLm?‰Dž?‰‹?îoµh	Ý,?…JèËIÙ­?n3ö3ÆÕ?^ô@G?§#ö>*T?"¡eüð<O?`ýa?™?»JÒà?e¨â¨§a­?kd_[sXé?£j»Ô¶W?˜Aƃcu'?îB¶žb+C?©EÆî©?€»|͘ë?ŒÈ‹­D\«?§¥¶èœÒ'?¥lÔg~?î¥^|j½?™
Ÿ¢]'¡?";É­ÕÞ?ƒ]Á¨‰¨?ª†å#:)¸?–9 2:â?ë?©Tý?¢»Î#D?€ç"Ë?w±ŒúÙ¶N?ÂDùü}?¢u	âïÞQAGN4FGL J1216.4-1358?ÚHqL¸.I@HŸU›=À;&:Wê£À<…AøDJ@ [&¤«@5ºÚ\‰?Å}®ˆ*Ü¿|8ù" Ðý?¶POx¹$N@<€;¤›Ö¿ï·1Å?ï îؐO?ÎH»…§ŸA¿çviéпïø£NNB?ï인KhUNASNone?ï¬b=P²9?€¢¡é"éÂ?Yë
úDwO?V  ¡-1F?ª泌å?~±°6Ö¹?ïѫ筁a?v.û{ðì?JBæk€O'?Wr¡¶%?sá¯^8ò?rßaR?îŽÙŽ@
ü?—­»©R¸ù?ˆÙ
S?ŠOׅlÎÑ? Ü%ÚU¬?"Y!s1ã?8A÷?j«Ë–[š?^ùRÊѤ?PcRtð1?ƒ»Ç¥FO3?g±9†æ?ïDäÇ?'øÿGòê?p'8Ñr˜ã?iU¸´^d?"?è°ãJ?'óßÑ°c?ïc¶a?švßûë­¿?Zé­nÃD?hË÷ä?'ínnLØ®?™·F¹Þð?í×퀇µþ?žBç¥#?‹íécAª?‹—0ƒ?«»lwR·?š•>QZ¡È?ï
3¢+'?ˆ&}Vè¦?oÍp]K¿?iµ?Eoàµ?š¿ñáÈ÷?†Hm	Ì:3AGN4FGL J1216.8-5955¿ïžB®®Ý+@>ØÓkLÀ9bsýþžÀ;%‡\€3—@/ÛåÄj@¾S<½öp?À愙WT{?Ï{£ºY؎@9[Ývh<@èÀr×
?áRá"öW¿áôÁÞ\A¿è9Xç!â©¿æZÙ㐿îgñ`ªåœ¿ïåaHÌ"UNASNone?Úϗ(6f*?Á3¨6sE?΋¢üÕå6?ºÐhgk³?Õê—XKÆ}?ÀŒ‹ßFÌî?Н"H,G9?Á/µOX?ËF¡3/Ç?º,ÇàBº?àߕ§[?ÁÑ£ê3¸?ÞpÔ Î
·?³%~¶Z]?Àu7.ëOð?¥z^'Ó?ÙTÇ¼JQ?²YžQÆ8Œ?Ê9ÒM"?›¬è‹,4
?Ë+ËJŠW? Kš*Š®t?⯾ÇÙüi?£=zÞ*?Å(ˆPWA—?¶/Å6%?Öh.SÇË?Âs!¤"H?ß°©€—j?àoGfz?¶qK"C—™?³ÛÊý¥îÎ?Ñ
Ï±Ù?Ãå-
Kº`?ä«G¥õ·A?Äí¿ªi?Ï'b«¬þ?¯Ý¾*«Kß?Ďôá$-î?ª!%±ÃƏ?ãøï	E?³3ڏ¥qa?¬GÄ?ً?ˆ®¡Y$¶"?ҒE.¼›?ªônoH™?äòa$™M«?ª*݈¸ŸMIXED4FGL J1217.2-2500¿àQÖs-ò@B›ÿñÀ;k$á`؈À<Ô¯«SÖA@¶E‰÷æ@>¢'vge?ØfÜ­ë`6?æ—r½·±@
›©ÄŠ,?üüøÔg Î¿èPä>X€J¿á Îï¼¼¿›à®^«9³¿ãêv–_Rv¿ïÿà•V"¿ïÁa)ÃÂUNASNone?ëóJ<0ª9?±Îe'qêñ?´‹'‹V?©•^ëU ‡?¨¾EÈT? õ"¿82Î?éÒ
Nc?ÁTÌ`i?ÁÐpærg?¼+Œm-¢?³n—¡  ?§Èt7/M=?êŒ)	\Á?ªà*Ò°tN?´Á•a"¨E?¢8ÆÆӂ?¶Ý"U¹q±?¡ß÷	?ç?"¼ hg?¥Y:"ô?¼`I}Ï? ÍO¸%Ö?ÀELÆV—?™•/Õ?èÆjdº|?¹–é‹ÖU?Á…»©—q)?±žµá"?¶Á5ˆÛ­Ò?­-BLc'r?áÁ‰ÐMà´?Ë£>±Êž?ÒÁ ´1?ÊÙ+Ü8
ð?Ãw˜µ:S?·'42}$?çšY''?±á…ä­…?½"Ž(2Š?¨ dsy?Ã
ÏtOÀ?¨®ÓË@F?Þ´¡=¹T?²Á¸ŠŠ,ö?ÌïJP0D?²½™ðÂÐi?ÒÓ¹š.Ù¡?°åkaõSÚAGN4FGL J1218.6-1049?á°òA.&7@Iœ,ÂãÀ:´'QžXÀ<L#{/KG@ؓ…ƒb @ßoijù—?Ӑ¡7óŒT?á6,­4¨@ó÷ ]m™@áÞõnW?ïÿ·hª¿Û'{°)©¿éhÚ´ìÜ7¿ð?ïú—á2µ_?ïÿ¢bôUNASNone?îÉ5ñ~‡ð?Á=@ùցh?RTc…'Ÿ?n\ja
BŒ?¢ÙýÌnå?Á2Ì	9\?ïk3âL?«qÝáô²?‡*œVzo?¤"Ô72?'K[ÇF¾?—i#Ðý?í1òÕ0YË?¡‡@ËŅ?œoÛ	?•"À×ó‡Ò?®ß› K\Ç?œÙäeÚ?ïÝÂÅÚ6º?eäSæTÝÑ?(éj Å?,Æu?m¾?pWQªÕq°?eJ2žÐʏ?ïƒ÷]'x?›ø¨µÐ¹?bâü?wK:ÈG;Ý?ŠIiƒæϹ?™R¯Ú‹—Ç?íãMgð\Ò?¹vz>Ï7z?–yô©-âò?®b\èú…?¦Ž/(ó¥e?­š!9A²U?ì)¯Ë›[?¤""Þ#*_?ž
¸äº3«?"¹'¶À(Ì?·4¬J,f>?¡"Ê¢
?ï?è‡à«ô?"Î@=¨o/?Sµ©dNÉf?`ÊÂ÷'ù/?–Ç"o1gá?"=߇ÛAGN4FGL J1220.1-5558¿ïåFM8ºS@ŠŒ›"UeÀ9é'Dé>À;î(«ð´3@ßG`'»)@µ'-lJ?Ã+þ +ïr?ţܾ‡d¹@Á\ºT$@tÔHD:?調.%­¿äëEÉ7ìÖ¿àÒÿ¡‹U‰¿å(‹¤äPw¿ï±‡¿g¿ïýyb—yÚUNASNone?ê…h5YºB?´3ð!A—p?™TCĽï?"™ÔÏf	h?¿ֱÊ_W?²9*þbD?æU'€2Ñu?ˆ»¢ê?¡~ÃF¿—?¢vڔñ?Ñ2Á'D?Àd~Îù3?í9¿á¤A¶?ž.ïŒ	?•µH‡êUÛ?ŒÙ ¸O+?°Ä®Î½›_?™‹žéo?ë¼8pðê?'bf:̤?¡ ª%|?|ßIè['†?¹Ž-¢÷ý'?#±Ô܍K?冁6KkŽ?¿õÙ¥<(ê?®›Ÿ]qØÝ?£E*C¯Þÿ?щ§LúH?½ ;oþѾ?Ý̐ó"ò!?ÆÛÃñÃ–?©Ô‹…?®‰MédT‹?ßT{#Ú?ÅaÞí5Íí?éQ¸8Yý?®Üžaá?¨çÕ[ó\?™MkŸg?ÄÇ֘Óv?ª5/•L‹|?æK—
ў?¥·s$^ø?³FÓ$ßñ?–m%{W?Î^.:OÑ?¢À pW¾ÉMIXED4FGL J1220.1-2458?ÑdêüÉÐÕ@B­³Ð|"¶À:œ€šÅÀ<c«Ø`~Æ@ _ºª@TXÍ ¯£?ÀmÓÃ-¿‡<3•ŒL]?Ȭ| 9›Ø@Iۂr6?ë|¿€^	¿ä)ôÆ)¿â<½ ‰ø½¿ÜB_ !¿á¡–
W¿ÕM!ñÂO›UNASNone3FGL J1220.0-2502?ïÊŽ°÷?x±~4Õ?U\›«§l ?U;yäÚª?uœ'ÊYW?sé ö³»°?ï¹8bòél?urwˆL6?Qx"À8-³?R\–ÓœlÙ?ÅïêZf?s+Z*Ô¤?k§:c?u.–>þ?[àåŽÕ?B¼žVÄ¿,?Š#jH"x?t'ó':(?ï*Ò<+?qšÜ榌Ï?oéÔ8á¦Ù?K½`âºoé?–¨}ïi?q"öGg™'?™S´Ä?x@J{)é?fâ<"(Ÿ‹?X»HÑ
5A?…'Jšùƒ?t²F{ÉÖÌ?ïQ×Úá§>?Œ66õiáâ?^D*Áe‹®?cÔPô‹l?"àÁú jz?Šhå
 ?ï	óÃÓ÷0?†›h ±Ä?g·"à,$?Uÿ»H€K?›Ê"ëk?…ˆ4÷–k?íh1~l|?ŒåՂ4ˆ?‡^=¹N3Í?m`ôÛ3jÚ?±Ò¬Uv
ª?Ž
L0êŠvAGN4FGL J1220.5-2745?èûYuš¿g@AMçê_"ËÀ:zÉۀĶÀ<>ðd‰Ø@wQ-=¿@¨tBÇû­?ĕeTB¢?¶Ñb?ïf þ'@Iòµ>»¨¿é­ûPm׿Þ†nCªz¿ìbÁì!¿Û"fy±œÆ¿ìÿ»Ëǔ¿ïÿ\l¡UNASNone?ïLwLg¸?£¶T$€?}$r 
h?‹:îßä;?ŽJiGˆö?šÐÞÜ8C?ï½´ÚpÍ?yd?D?Y—ÙÀÆH?aʃ^&Kx?z¿œt×£¯?rÿüíîZ?îú²…¼?|ª¥¤w–?ƒ©ÑćÁ?")¸cö?–ÔÆzÕ£?†ÿ
{rÖÑ?ïd{RJ"?oRs8ˆ'ò?{ãÌYf¤?_³â<ïù8?‰uo?iQœ?gTcÔð˜"?îËtQ
µ?˜ðwŽ±?‹RŒ@Ÿë3?"}>é ŸÆ?˜ôKL÷­á?'¾2"ÍŽ?ï3
VΡl?"¸Dü?qhj*½¯?{<v.¼(?•D´1‡?v!÷û†?î§i»Ûc?™)Ø#?'<5€²›?‹*'¾Q?§HÌñŒ?"ðP Üwó?î>ñ§o¨?¢‹??¯8?•0²Îû¤?€Þåùx??¡xÛ1_5ª?…v½AGN4FGL J1224.6+7011?êõD'@GaFÜ]cˆÀ:\H»Z´À<PÑæAq@ ­'ÐÅ@7ºœH ƒ?¹Ð­'ÐÅ¿¡ÊžÕ˜£?ââuuÍâw@]/ÆO?ïÿ
¢q›¿æFIlÊ.¿ë ²Ý¸Wu¿å¸
ñâ¿ã8?!(οïÿøþÙå9UNASNone?ï®"I¬$?­Op¸qB…?€»Ì—}&?­V,"UŠ?]ôvü·ÿ<?V+œ7$Ð?ï¾4îk¥b?y[ Ìü
?Uð¡Ðq™?`<Tb¹xÔ?{i`|¦ž'?sɋlϨ?ï)‰*$†?…ÑOcKœ?z»1ü¦.?~7Ä£R®?˜l'èÇ?ˆT)î~ó?ï©
ãËõj?e`»D¡?shy¢–Š÷?\ö¹‰fÚ?x"u^ü?YTϵ<fÓ?都™ÔŸL?"M'™ì³o?€µ¯%ÿ7h?'ù5}÷c?d'©± f´?e%BõÀw?ï8´ïWކ?"9#ûh ?i4ëʉë˜?sÅ}Šô?•ÂğÒyÒ?'£½"¼Z?î:¼íÒR?–Zô˜B×k?‡ZøÙvýƒ?ƒ¤ ÖsB"?¦}r÷Mƒ?'í‡=²¤?î¾QyÅ=â?‰Çsû˜?"¢w'rˆ?…ÜL¼ß?""Y3"3?yÃ|žÅ/AGN4FGL J1225.9+2951¿ïê/Ÿ¼¸@Tñw[0À9'7 þ}IÀ<@̺XV@±È,)(Ã?üT¤MQÂ?·JRŸ	E#?Ú÷FóÚWÐ@"Ðàm"@±a5$$"?ï•¿,{3?ÌïÒ Ì=Ü¿ÑPLH­î»¿ÝΌ 6즿í]¨QÃA¿ïêo_‰RzUNASNone3FGL J1225.9+2953?ŒSˆdG'?Šoqj
Î?ïI'92"??"ÈnÝó?b©™Ê•?‡'ãº+?¼"$‹-MÊ?Ä*†‰Ø˜?ên-kYP?Ɩt"^6?°lp-ï8?¯œ©[ޗ?²7aÕÀŠ?¤78KW©?ë5‹ì̋M?ªÕLg֋º?´?†¿Š?¡Å]ƒóýÚ?µÞÍÒǒÅ?šÏܱ"J£?êXþ㏠?§T˜š¬nQ?¹vj6‰ç»?œ©^]®[ó?'þ^­C÷O?'¿Í¡8?ïÇ~&Ä?™µ|; #?…Q'B~Äp?†´œeÎ?±•B"j®ß?Á9­¶1)ï?ë¬XÓÞå?Ƹ‹í^'²?±ý-öYú?¶žv_±**?¥VEèÄb?œq*a=â®?ì~:R6Y?¥Ï"Tõ¿y?±`Ó9Ú^‰?Ÿ¸ß9sڑ?ö'îs?‰ÛœA¿"?ëFvÇ\ j?¬OÂ5<g?¾NÀHÓ?¨#š^Ç}ÜPSR4FGL J1226.5+3023¿•ªÄuv‹@TéªÍžƒäÀ;A§
›duÀ<x
c0Q@S͍'ùg@ÁòÜ+¢?Ì¡›†-Öþ?™]g—Çe?È01¡Õ{@#r ÜY¿ë^¿¨÷Ûn¿ÙhòÝ­š­¿Ø@ãȑտëÞ
Â5o#? æPž`~¿ïÿ›¡[¯ÔUNASNone?ïT92q0?'Üo#-¿?]¢›Y?`aÈ5ì?"ž´$yë?'ÆÍzê?ïž#ÆG'S?˜š¿ž
ùu?U·«Ý¦Õ?`µµbY²À?…Ö7i)¸?˜$©•€©_?î3Lç?"'·='‰d?xâ^•@?{Œ†kSˆ?£®ñ´Q›?'Î}—~Ž?ïqݘL¦?sTóâº?OªÔK´¾?Bz°'Ž?ÆöLŒ›e?rÙýÙG?îT]¨ôÖ?¢Å>F¹W7?q¢ZW~à?r!Xõwe?¨…ì9_Ù@?¢æ;6M?ï,We±O?¨,pjYË?`"85\ ?m{$`tñW?œ(ÌC*›?§Ïgè¹ÀÀ?íd±¨PŽ?Ÿ›Š>ðœ.?…^²S¢N?…Δ?k'?²4/× G?c×»ŸE.?î¡žË³?•E‹ÓÇä?fY 7žùê?c
K4"#î?­Ù«ÞcϽ?"ÝáxÿÜAGN4FGL J1226.8-4907¿î}+¾ŽŠ@+ÄÞÁÁ×À9}ÎéöÀ;PÜ¢b–@	ÛhQx@B Ž€a?¾ß¡:ͱ?Ç=ýçvò%@H™|=h@@
EBÉ(R…¿íóû¶Å?ÎâüúgØ¿êO"J'°¿î«ØáX&¿ïú	.Îõ?ïá c¸6=UNASNone?ïÔîLì\?w/©'î?S·"-ÒR?XSe".¬"?pšøŸ§S?t$Iò0—?ï-dS2? GȜŠ's?Ÿ°îv ?'+»Oí3?'uëf­?–DÎùé3·?ìiâê›iÓ?¤¿ ÅV±?žõ-{ÿ¤?"èAøfç<?µI+]Ÿïÿ?¡éíÚcŽE?îCẫÉ-?'Û8A'!?xæ t0~Ð?b"…Käo?¨¥H·#Ï?'ÐÕ±\`?ï~85îN?µÀS³)?oSrçÕÇ?r]]ôgôn?ˆ BÝΑ?Ž%±»/‰?í£FÀüŽ?¶ƒR››a?—åYdc?©ËÑ\ûïÕ?ªB¡D›«ç?®˜º¦jÊ?êÎFÒò?ªò"«R^?ª%J»…¿­?®w'¬Â ?¼{*BÉ©,?¥³B¿Æ"ž?êü"{Lt?¯*…Z_w?"$ß~lŠ?"N6¬¤O?Á«K†æß?­óä€Ø"AGN4FGL J1228.0-6918?ç¢H(ÛÛÀ#âOëОÀ:ÇM~8DÀ<)©HcF @Ùe4%m@o«Ú
ýð?ËT3]û]Ú?»(‰Œ\`?ð•¢y<,?ý9+€À…?íKT'
`ç¿èÿ §?tŠ¿ä|<& ûù¿ã.÷ϯÖ¿ç…ý_çœ1¿ïŸ€-·É0UNASNone?ì‹-ØÃ6?µÜêÑ­wÁ?p׫vY? KÖVßí?º¥šXÜ:(?´—ÈÌ÷Ð?æ	ð(5m?¿NpL)Šy?€TK¡1,?'¡‡7	/?ÓkMÃy´C?¾´[/VT?íQ˜s U'?šp
Ôð1×?€e#Û?s/ËdäÑf?³fšâX ?˜÷úM
¤Ù?ìÚqäQ?ŠIEöÅ?Ž{ê\)̂?i¡k*±]?¶¯%X:e?ˆäåSsñ?æªÙÀÙ­?¼ÚÇ²í¹¾?x;A`þ¶"?n¯Ì%u?ÒI_y& j?¼©I¥e·?ڂL9¥¤?ĝW«ÚÜ&?ˆr~TY?'˜b¯D3?â]-áe*?ĂUB°1i?é(ðÜ÷gU?ªw}å‹?'ÉûQ¼Ù?ƒ¸5Þ®?É,¸+?©_bb·	‹?çÒ¢œ?¡ÓpÇ?¡ŠUs˜áµ?†Iâ-Np:?͖ à\Þ?¡YPóöLòMIXED4FGL J1229.5-3048¿ßzÅ	A0@?Ó ù	kºÀ:óD{ZrÀ<e†Üþs@âƌì¸@»œ"á?ÖØ­Áä}?ÉäbÈ!?õH(¨•µß?ú`ŒzLL_¿Þ)Q¨,Y¿êR½<6¿Ûœ²þšz?¿çEa-¡¿î	‡"s\¿ïêvUNASNone?íz°/ˆ-á?¬ßø«Pdí?'Æâ_ؙ?wÒx¬
ãa?²…¨ƒ!?«ÝIº¼²?îü Æ1[?"{\½|??ƒ‰ve©ÔX?€RDÉp:g?–§D–̤x?ŒË˪iɾ?îû"dn?™ÔÅJ¿š?–FÏ>÷?ŽöÚÎ~cï?¤­C—õÎ¥?'¥o¶}GW?í{î¥a?ŽÙ5+ƒ?'kM3˜‹?us™qTýÅ?³9MC¶«Q?Š¯Ä¢€?éŒ3x'æ?¸ÔQPŸ?'P×ð?‡Å¼ˆ$ô?Ǐ(ø°Î?·msŒCä"?í>?¢œ†?¬éJ%Ðå"?˜Óê¶2Oµ?œÎmGs?¯²|¶Â?¤þüôؐ˜?ëûe".u´?¥¾l݄ó?¤ãÿÇÛR?˜6}:?µ³\ð–¸?ŸÙÀÝ©™?éôL G§?§aŒ@i?œ2¢Z+œ?®>o»õp?È/ÈzW´ó?¥BT7Š'ÜAGN4FGL J1231.6-5116¿Ïe¼ðX:@&÷\òI^À9ZZ¦>ÊÀ<z>ŠJ@F:ωÀ‰@fû_‡O?¸4€·å#?æj'ào–ç@'•€^_0è@¾€JGÖ?ïÈÜ}Cø}¿½Þ½åÿ"à¿äw݇/3Ê¿ïi'2t¿ð?ðUNASNone3FGL J1231.6-5113?œqÜñp
Î?«Ìàª
':?ê/ÖEá$Œ?ˊ"Ÿp"?òkJ"f4?Ɇ™a»[á?Ÿl¾Ža%?³å@S/½?ì`LU‰?½L3¬Ð?µ$D­Ùír?µð«ïʍ3?Äq'ߍ'?«~ÌÕ)ie?äNãT"ë?´'¼Alä?ÊSTÚ"Ã?±â6Ó?¢3KžôS?¥MãÕÖJ?ì4¿x.ž?¡ó4xT:ð?µWê—uîh?›†Ù,ê_S?©áՍx•?´ÂêÁ?é.d¹ý?Ìû!˜oç³?ÄÎ&KÀ4?ȁ\k»º×?™\qE­?±þÝL¬	?ì/{xúÆ8?Ãañ33‰?¸D
F}U?¿ËqöðëC?½¹ÇÕtĬ?ª¤>ýÛ|W?äÝ粉Þ?¹]G.Tá‹?Í«}K%I?·	*&«K¯?{
l¾?n/úòä‰c?ììï}î÷?¥³üÌf?¶çåw=¤%?¤šèÉ7KPSR4FGL J1231.6-6511?çÀ­Ù©TÀ6Ÿ~µè…À96‰@†
À;9åèý"û@ٝÃõ¸©@"dEú¶?Ân D2Ò?ÝÊBÄJÈ%@ɝ_÷·\?ÿ'—¿ïÿÿ)@k*?ïÿþˆ0»Š¿à¿"àT¾ô¿êŒ@À}¿ìý¢yM¿ïûîיåUNASNone3FGL J1231.7-6513?¦Ï»&¢¥3?¹ÉŽ5Ú¤É?ÞÑS«^ú?ÏˉÁ4h<?ÞT´ðªý?ÏÒ3šrmÂ?¸%2ö× +?¼e¨a™´?ߺ:þ"Ð?Äïk]F,4?Ú<xDE?ÃÀG§Î)ˆ?£AøDJ?ªÑ,þœÅÌ?áژèC˲?µŠb•²•z?Òù-¤'6?±QQj >?Ãο­ÌÎÈ?›€Úî¿	?ÙÀ´˜
?«Öƒm6'?ÜWëÿŽ?®Y×Z‡o?­qä8Æì?ǙJ~ÔFi?á.]*8Ê?Ð	I?Ùõ'Äi?Îêìl=c? \JÛOÚN?§óÈAç?â6"Ìáx3?Êm嶨ž?هm	÷-Q?Éê
5®É¾?²
¬±{? )EËE¡?äDX	´è2?¶¼ö}x»M?ÒôŸ@Äã—?´9†ó½?°7כ}Œ'?°˜"&?ÜBv'=\'?¸)ûBX©?߯"–uLÞ?¸Èü†l…MIXED4FGL J1231.7-6653?ꈛ¥7‡ÀcËďªÀ9ðh¬'ÃâÀ;G¸ü5p$@ÕúK`%°@¥EŸF'?Ô͍Ý"ÛL?ãÂÜSRl@	ôŽ:!d@!$‰w7š?ÚþcGοågÔôó¿ì®Êžc˜¿ëiäñÒÁ¿ð?ïþ× ¿UNASNone?èÎwF§|?Â6Â[k?·Û;øB‹?¶(a†`_o?ÀØ 4é@Ì?º\*DÄw‹?ã.‰+s‡r?ÈYáȲ`æ?£ì_åóÙ9?¤ÙÀ]ûI?×%a¬uòÔ?ÆÉj¾K?╸gÔ¿N?´¨Df¾#\?¸J¼º ›Ù?£Àé·
»?ÔÁà)m.?³ÜWQõ«?ãPõ*[j¬?°çVL#*c?»¢ÿQŒî?œ-Õ~¶º?ÒuU×øÏà?­5'¡cÿ?á!ØÊSm2?Ç°õ=@A?Ëȉí»@?ĶWÜF"µ?Ï°è÷ ?Ãv«zd¢?Ï÷ËHhNž?Çs­ZÛ\¡?º
üyÛÀ?¼"…ÈβÍ?äÀMžª‹À?ɇø~δ{?ÚâÕèZÔ?µbÍ̆hÖ?¾ö.TŸÑ?¨aWAž?Ý_ž—k}8?·`+©p	$?͹iÌ*5?°?¤&T!?Ìkí]Ѷ?±ÄÁ‡Ñƒ?ávª6õä?µ‰œ<r]QMIXED4FGL J1232.1+5953¿ÄMÐ*ØÏB@L‰ÄڐïÀ;½—¥¤À<³Ùý7@õH&4r#@	=·ä{õ?ÊÈü]´¿®RºÀŽX¦?ÜüϞä1B@v=}dá¿ð?ð¿í9~¦Ï¿ïÄ_@¿ï0_y[X?ïGâ¢w
ÓUNASNone?îțÚþ?´ )Ûº‰?p"Ï|~?Žð"PËä3?¡e´D'½­?³šã"×è?ï•qKF%?–—"`î¢ø?oDá<¨^?ŒøÙÉõj?'Òtö±Ö‡?"KwMÅÙ?ìEÞö3è?¦Ä¯¢é{9?•»Z?‹?'Ûêê¨}?ºâ1@]?¥¯¼X¦ÙJ?ïÛ¶@ˆ8?]qØ'Ñ?f´ ÷×öu?YȪ{‰?[*=cc]?EòGü0?ïp‡®yig?¢UÚSÓN¸?s¢Ñµl™h?Œh–ü¸ 8?Š«.iq? ÂaèÅ	?îÀò"Û¿"?®ã®è¬?ƒívæfPí?£#Ôޜ?êòèœ
?¡±œÃæ6e?ëb-É;ô?¨`Xžæ…?•ø
]éúŒ?'éD%¢Ú?¿q;ùÍ®A?§Dñp¡üà?ï|${Šdó?ƒ×²`ê@p?"t¶S˜<O?€Ã°Þ§?yU—¼•·?l‰Þs¼ÝæAGN4FGL J1233.0+1333¿ÁVUÑ\˜K@RðÞÑ·À:ü˜lrðÀ<B½=ã^@&Ø,ý9&@§ …±…I?Ãd´ CŒ?Ìf7AŠ¹Ø@ä†&ö@Õîßq??ïóçÞ¡
§¿ÖŠîü!¤¿åß«Ì¢¢¿èH'_ì#տ뒥2.¿ïñ">¿UNASNone3FGL J1232.8+1332?îÉtv°œ§?"vš¦ Ê?õ‡X‡×)?uՕv³áP?Ö­wý$Ÿ?'d™•~1?ï*Ñ·›5?"œ1ËëU˜?€ÓDκ?…æ{Ú??'<&¥DîS?Š·f|Ê?ï`µ!Ši?×—oâÖ?€¸¯;ÈÕ0?}…ð—ô¨/?—'¾š4=?Šaz›0?íʨJ{=?†Vê/y¹V?¤†¾àñÕ?'s¼ïÃʀ?š-9àP¬?v½¾jsF?ìàBµS«Æ?¨Ô*(òµ?˜˜³‰'Œö?z|Õâ¢?²×½skò?¥w¨eIT?í½¦Î$T?° ߥØÇK?•ÿRT7o?¡€]xc?©%é÷›¢?¥¥ã7Ÿ?íØ׺z?ž†g­Ó
?"¢øÐÒ9?ŒSW»´¾¼?¨å2ߦCK?˜®dkŠH¶?ê8o"«.J? µvÔNŸ–?º%ï±y?v/?c?´gû'Ü6?'è@6/ßAGN4FGL J1239.7-3455?ȵìx04É@;âbS—À:ÐDñ¡˜lÀ<Bãü";@äÊ-
O9@%1"Éÿ?Àq2GOõ·¿³d$í ,?ñËý™ô2@Y±=¥'?Ò
»Då_¿æ¦F…öN¦¿ïÿô¬å¦¸?ïýŸêÁ¿Ñüê
î¿íIhÉíõ<UNASNone?ïZhr@uw?ž$Xjsh?€ßÙúqȈ?™"_à5@q?ˆ†	ƒ‡?—?Š3a|'àó?ïÞèá³í6?xøÏ{Pì?I¢í!«$$?hâ–ôíx?j®bô¬è¾?pùÂ$Xt?î½H¨îÕ? FkûúØf?eKHƒ÷xÌ?gõøžn‹ë?­ïvé-? %ÓòWŒ3?ïì$ê¬Aù?Zâz;¸ñV?0ÈÏ;|EK?0_;NàÊ?aÁûh»³#?YÍýOÓ?ï%5:ÄÇ?£Õ–žà?|°¶³ß?¢±ÎS;™?‡§4ØfîS?ŠMähŸ?ï¦~‰ÈÁ$?HuøÔú?YÆé]ý?-$ø¢?ƒ?¤¨dçL?ƒ–`Æ딕?í»"0«ø?œ©.Ü
;æ?xL†X+µš?wpĈb"?°ŸÙéÉe?œ$"'øi?ïªm@°þ?ƒF2‰S%?g#ômyüØ?w̖tâ²=?7wÁ§²?~Ô`éq—¡AGN4FGL J1243.5+5311?ïûОœ}@Oñ\(öÀ;´vTðóÀ=C'üÇf@ cõpÚވ?þ*(,nô?ÔªL¤ô@¯?±Ž%È¥j?ÞzÊáæ'@x8֋<Š¿ë$ñ`®—¿ì.û€"dü¿µ™ÆÿÈ"¿Ô*¡OÆ¿ïx×ì;?ìÄs'-Â0UNASNone?ïªYí~•? ­PuWRÊ?FOÊj.?T;öÀ	Ê?""Št6U? všExö…?ïÁŸ:K?ƒœ¥8Cs^?L$÷¼g?Xm˜»ùlõ?{ >?¨ü×?'0ä¾Îä×?îðAµÆ»?œm¿Û~"¦?ë ¹¢½I?Ù´Yüø?¦†3¹ª€ÿ?˜²·é4
X?ïØÂ*ÿªg?Wƒkµ¨¿b?D©«Þ^P^?3—dˀ?q	µfäi?U¾\8éj7?ïg¡
Àè? 1ÚéQ/?Q4'àCHh?R+·YÄ$±?'ø•'ÛO?ŸÞ"xâ!Å?ïG'!_©¼?ŸFò²Ùie?`Œ"gù?zþ—EÜÏ?•ª·kj?›xmËè}?ìâ
Ýýæd?¦œ|ÑK‡?Š"àS.© ?‹±D¹ þ›?µ=,?¥՘âà?ï"é¨i"î?x"†2?T¥-bïýi?QÕG¶1>?Œ0ð>À$á?wˆO6ú^AGN4FGL J1243.7+1727¿ïèjÃJö|@T
¯%;À;9@À<Ù$H¸@ ‡Z$ää@\ú&¢+9?Å´ØÏå[¿¶9÷GŸ¦Ï?壼gú»?ù"€€Ce¿çGìþ›{ò¿ìDåýö:"¿Þ5'm,S¿Ø쮿p˜Ä¿×`^l¢¿åIÛ¶t›³UNASNone?ê7ü‡qñ?Õgé+ä#?Y2|+¶C?rcýBBë?Æñ'Ùý{°?Õcv•f6É?ïK$¥v"?ŸL©•©ä¯?oér 	/?€zâgW?'ž?Ÿ÷«?›aÙ0&q?îd"®èÚ?˜é\ûX¦_?iJn'ŸŸV?oýÁ>Ö?¨#3/¾p?˜§ûtäf?ï\2t¶$?ø/…Ñ?s;•-dA?`µ°ãü€ý?›%"kÑc?Ê¹T{~?éþ˜Ù%/?ÍF!¯I¦Š?lÐÊçÔö?sP%$¥9?ǒYo™&=?Í*‰ˆÌº?îQ:Å£¸¬?²òÔ'<¸?zœíf–Q,?Šõšµô$G?§˜µ÷{՗?±Üú:,ò]?íQ½å~I‡?¡U
¾þ"µ?q 'ýpë½?se˔ÉP?´XT+¦L?¡
}}?'?ìÄ¢dw?£Þýò?'DX¶ö-?…bË+z?ºÐÖŠqo?£
ûâAGN4FGL J1244.3-6233?ëÉó˜Wi?Ӝ?{Àë˜À8Y®4[Q_À:Žž @7Û@&ªfpwa?¶Ž±3>F?º×Eâz@ÉÉã
€ò?ø8DD}ˆl?ïÓ5!	†¿ÆgÆ£=q¿ãg]Ý*é¿æÞíášdE¿ë›@˜vƒë¿ï.
ß¼"šUNASNone3FGL J1244.2-6227?ÂÂe±›Õ?¶ÖÒ_ Þä?®¬4–~"Ø?©'¾<G?éd£J>ßÜ?»ôÝâô¬e?­x~:õG¶?®Ö¶Î'P¨?ËÓo,¢d2?¼'"ê>]ð?ç3œQQMÈ?¾
–Éõ?Ç#3bÐ?«VÕ´-íÅ?ÉÍö˜x1j?®>j?ãÆù˜Kª'?²!AüÌ/?¹ãÿa}&$?"ZÒ^‡î?Ïh*Å©ö?¤>HÙì?äéu'žð¾?¥ºÛÎ;o"?ºÄF"p¬?¬ƒ¹Z£š?¸¬ÿ—™G?±‡~À·?é'×HÚB	?¸Ì5*tÁË?™îÑ肚?›S›6ƒ?Ë!NFŒº?Ãuil2á²?èh;‡âÚM?Ã:Š™»AN?ÃkxÉëF?¨#PfD¹‹?È^2-'LÔ?¯úQ˜¸˜ï?å%˜–lñù?³jt˜!W?¡ãiÁ@¥Ø?ƒç𩝶?ÓtiˆH¨)?¯žp,³ž?å'"Ÿgl~?¯Rq>–±OTHER4FGL J1250.8-5424?Ó«³fþ@ î)Ø@žVÀ:ƒø³o.À<Ï<é•Z@¶Nií"@qº?À~ÀzY
?"0'—|<?хX.•>Á@•x´Ðì?ïÿdd-§¿ÖЏ$Äì¿æ8õ³¿Ù¾@Bo	¿éŽÌܽ¿ØˆUg"UNASNone?ë)qWÓrü?±L–VŸó?†–c¼èÔ?>ñT<?ÁðÚ[‰FC?°šÀºÌ˜j?éðòïã?¸ðÛ*.?{l"^Þ*˜?|oӋф•?Ç`ÐÒbZ`?¸Bá…ÎN?í;iì
ˆ?žf{c¿©?‡ìƒvl˜Û? ØÉ¢yQ?´ø"AÒ¢?›Ìâ"GÉ/?îv(
‹W?yÿ)²R?zÃ%ºgÛ?V׬֋ˆ!?¥E¡¢ï²?wóh¶Ð?å³AØ´ÙÞ?½O*†L›ö?'šK&aA"?‹DVú
?ÓoכTQ2?½ï|,ÔÓ?âÁµ!_v2?ŦbsÏ?…
ò½Æ?\½g¡qL?ÙÓõD)Ž?ļ2Slí?èƒîÙßQ?­ð:»íËX?›ßä§k¶?Œôÿ­}?ÌUó°ƒ?¬E(×yI?몎5&AL?"+y¡Í.?'æŽL°ô?ua¡(+߬?½ñêÂÅÑ ?'ӌÂaAGN4FGL J1250.9-4943?Ô"Îíʄ"@*M~Ë·ù×À9ñ¿³ß•ýÀ<8#;nk@'.íÿ"@ÿCB?½jtËáY?¾ÖÜG©ã@Å$aß@iˆZ?ë†+'Ëöä?ÚAžlK¿äÏ?mÔñ¿Ñô" áw¿åˆë–¼o‡¿ë:ÿ[ë8UNASNone3FGL J1251.0-4943?ïÕyiMv€?döë(â]<?LÝ&	T§?DôDï ò¶?q§¦‰)|?bE!Õ?ï£UrMOi?ˆzÉD¹	Ð?`˜P"hó?iõAAˆ?ƒoßl?" Ìc§a‡?ïŸ'jd3?s3Ü3z´?\+.¿–R?UÜ ƒÞff?"¶y›™Æ]?qLçôJ\?ï³Òˆ!?r.øid?†ççïã´7?c†¥ò©'?"u'½Ý9º?kü÷9fI?Ì.?z»ƒJŒ?cµö=Qι?]T"¾­â?'QÒÆ7¬?ve_ÿ¶?ï·¬÷fÌ? PŠÏ)Ýð?t+œÃš?'w•·Y—z?šž#.<Û&?œƒœÍç?ï>ݬ ¸e?ˆ'´Ò©1?iö‰D9?hK/Ó~)?"åŠaWÒ?…Üj¡ù3?퉯Å鱗?ƒp
Ê¡^?*ò}½C?'»¯!5J?¨Ð%2ñB?…fœYKþAGN4FGL J1252.7-2520¿À~%¬¯Bp@B»ýq°GÀ:£9Œé‡îÀ;ëô9rè@"<͐Â@RoFøÍ?á¥ô@")›?ÕBTcY–Ÿ?ðèçÖyõ@…ë´½·¿©uy~Çc?áOmŽo¿èM_.cÀš¿ïqKÞ'ñ?ßÎùã0fz¿ïÿüÉï£UNASNone?îʙ˜[Ž?«ô½`+
†?‡6Æ>&üû?§úiiÛMà?›i×+—Ö?šU0~»x?ÍÍB?h1UpF?iò¹ÜµA#?z5+ó%`?"Z®ÀwZ?…ò#3æÖF?ì"	Š àé?¤>Ý>¼?¡=Ý\JR?–Ó$sµ€ì?³@Äüà?Ÿ(GT¤ÞK?ï†q™Ji[?y»È£‰eÒ?56«afq?2x-›×?¹é®†°?y̧k?î*"Z?©"¼7™Ãb?'[Mtì­?–pnW?´?¥o°D´mŽ?£~kcýà©?ï!óEî‡ï?¡wm¹…¶ý?tÂ(eÆ°?‹º¢jÝö>?–'
%yق?˜<7¹‹Ä?éa4ºê¯?®7ƒl4?±ãLÜ¨á?¢Ì³ºð"?Á‰†Í B'?¥ó³1u?Ή˜ù?˜;ÂpIám?Bl>Ï?QAj"œƒÍ?¥¬ óhä?˜÷n±Å}AGN4FGL J1254.7-4516¿×G2¢R¥@1—Ö[åÚÀ;…Y#‡Ä…À=gû'@ RTN‹Ô4?÷%
`¬B?Ö¶N›™y
?鎥.i@g›\è8c@ʈˆ¥*œ?ïÿá'¢±¿íä‡imP?܄",tþ¿¿)¤i+g¸¿èý0½b ±¿ïÿýawUNASNone?í¸¥õÝ?¨$L}–Šš?•Ú«v§ð?'`äD®Gá?©ˆJöJ)?£ÇÂr'ÿ?ì2©^øLÇ?·uïWêŒK?©)"xi+?¨žœƒpò¸?±Õò˛Á?°Ð|3¡Ö?ìÈ7Tˆ¡?¤Â'Íçcƒ?Š6"ÿ•'?"ˆ,p´`?²[·µD"? ¾ãAŠ?ëb(Õ`?™Y¸}]Ä?¨œAZS?Á\5â"?¸æ)[?"³<C{Ñ?ëmþa?¹IŽÊã²z?¤õ{ì°N?¡/qV¶Ci?ºQiÝG?µd²`Á+?çë"5·Ðo?Æ'Õ\z?¼ßš;ÍX?¾ihäÅçÖ?Áâ":B?½s8B!ô®?ê¹UbCRK?®û'Tâî=?£ÍBf́?™gË£ÿd?À'YÞ÷$m?ªõKVv¡u?åô¾j«¼Ô?°ñ´úÓXH?´ôœ«í?¦å€}ô?Ͳ·ÿº?®	,Þú/AGN4FGL J1256.8+5329¿Æ©D÷Á@OÏÞ灃ùÀ:A'½µÕÀ<2ºOò†›@¸b4þdt@@'w?¿JriÿÎ?´Å–¶eW?ñ~@'7|n@Ï&ݺZÚ?î!၏·™¿åPʽþÓ°¿ép¿ñ7n¿ä–fr•I¿ïÿ+Žúg?ïæG\µã|UNASNone3FGL J1256.7+5328?.k^"?€1ϐãpà?{ù-ø9£Â?y]÷U•Ò?wªºä¤þ$?mƒ'¸úÛo?îǐæuH	? Ôq—(z?Š¤=îjYÐ?"
ÒM*°L?™»Ä4úgø?"s^ÏG?îØ Ôæ®?¢oY"¿ò?ˆO¼îÂǺ?…ÎÁ_)‡î?˜ÄãE x?†8½—ÂØA?îμ½'y?÷ˤëɞ?'ë¹ÓÊÁ?x$79ù†?"Qî'ÍÖ?tH÷ÎÇ?î²CÞôd
?›ŸðU%?œ¨à
<?˜*À'mX?ŠHó®W?'ZZCÅ?í2ÊÏéÚ?³›$Ñ·z?›å
OGš?§sÝE?°'øȇ?©Leœ,•?í¸u>'Ú/?™ôô•0ã?—&QЮz?À¦@"?¨åƒ2<!Ë?'Œ•†+×?ër—a°õ?£ÅÎBþW?²J-xB¸¶?¬ÕOl½?²!yÇ«Ì?•¾ÞìlÌÈAGN4FGL J1256.8-1333¿ï?A¹*P@H¥VHþÀ;-Þ5ªÜ¸À<ˆK¹ë@KsÙ@¤@}= t.?Çè£ØaÖ_¿¤—±U±?Üí7OË@ëFƏq¿Ø/›#1ˆ¿Ø‡Ø_ñ¿ëk!ÃI@¿ÄÔèå‡-Ü¿ál‹ä¥0§¿ïúlb~Ð@UNASNone?úWR*?|òŠZd5?Ra3
(ö"?E±´¹ÞT»?ˆ[¶ª?{Ðq"{Ÿ?ïÑ̨‡©?odÍ«GÈ?CÚÈ®õ`?Jl(VS–À?tžR¼"‰"?k›$z	s?ï^p?G‹?~†h•°H?e%ÕwwM?Zr õW—?'=iËû?|ÛÖù·?ï¢}€´El?fÆ÷\U´?VmÞ¨µ÷ä?@Hd³¥L?"'ãñ!Wù?epÌÀ"Q?ï&¢Ë¾Ò0?m%%'j?bužhd†%?ZD')ƒt#?˜ÜòÂ|R;?XÃ¥+ª?ïsùÈø??œý9?T0×Tå[v?\i%r?=Îôm›Q?Œ,Ü*X†8?îܦ@"eo?Œ¶Jz-¶?qdJ
ßv|?jcJï9Ρ? 	·€·?ŠZb±'?îȌ­î?†lÖïs?së}:?c6Nbçë\?¡bià?…	庍ÌAGN4FGL J1256.9+2736¿ØÓcK¶@V+©¨–hÀ;äa1sÀ<£u»mÿ¸@á#õ[â@Š;WÄã?Ѭþüôã?Àå—IZè?èi®ðBô@ïƝޢ¸¿àf» Õx¿Õo"'`í׿ì•C~Yø¿Ô[€–é;¿ïýîþOü˜¿ïóöúUNASNone?ïÄ»*…\?›¬ZX¿sn?c$ºo¶û?~0Å (Ä
?t
l	Ë~?•x-ԝ¨Q?︢ÛÈú?"|}£¬?XW?~†rê?f´ÒGœŠ?}˜ïML?'?êÓªV?î$ TDŒ?Ÿ(½Ö"3Ê?'ª¡áµ?Õ2Sé¦í?©8P[	K?Ña4•?ï§Ðê¾¥?gÖªO?u`ï/(‡?^¡
=—›?wc6€¤þ?\Iæó#š?ï™ÁµA•Í?ŠoÒÜíh?rÛ·PÚ¨?tßHø†×Ó?€!¶ö¯ç?ƒ"iڇF?ï¬'MR¢?¥æIµ%;?o+ŽÝ&®å?'D¹¯ÄíE?›ûÕ]pó?¤…y­BB?íÍôÁD?¥ÁçÖ
tO?‹Ö¹%Þ³?‡ç©(1]?³ÞÖ¢!
?¤º€}óî?ï蕼P?†ÍT§º(6?Œ¨ìKVæM?€M
Ús%?ÎwëC?|¿iŒázAGN4FGL J1257.0-6339¿ØTbtá ¼¿éO0«¼²À9=Åté¶èÀ;nããiÇ@8¯ÿ;_@˜«B8‰´?†'vçh?՘" ;^Ñ@
à×ò›?ï,é™BS¿ïýð@o[Ø?ïÁW]ßÚ?¨f]O³¿¿ä-Þ)ìb"¿ê.^¸; ¿îD$QîàUNASNone3FGL J1257.0-6338?¹ڑMÉ ?·M󏂊!?¹9Ž߫?µOm®1À½?é¸+ö(ê?Á¿÷A?²ë#«%w?²´m¿dô?ÏYâÒüt?À5d±þ?åÌ"çÐM$?À¥Óñ{¥4?ËËJEh]?­Ž[ãU¥N?Ə$m!í?ªŽ<ÒÅêm?ãidSwÝm?±Œðün?½º>·˜)¤?Ÿ9,ù0£¤?ʑ»Q­Ð;?«Òvó0M?å¤IT¡†½?²Åç3ä¸?®cŒ@tõ?ª¯)7­‡?À_ÚÏ!™`?º(ïYáë?êЈ Óé?¿'ÐßoÖ?ž8ÈêJŠ?¡Ë­3úŸ?ÌåÁõG.,?Äè
üïe?çÔÉ;Pk±?ė-Æ.Dƒ?¿¼§)"æì?¤Nkxíÿ,?ÇCXW¸D?­cͶ¹?æ7•ßbÒ?±ÇÕݐÁ?¬ÓŽú,¢
?""«¸:?Ì[®Z#•?¸ç¥Aø°Ç?çÛyý‹Ë?»‹+éNOTHER4FGL J1258.4+6554¿çÄÌQ
	@IšÏ¿ÆT
À;"åV0Ž=À=%|'K@\P¡X)ã@¾Àdß}©?ÌÍ¢à•+¡?'wÿ&L?Ò%œq».@Æ-Ní¤¿ê˜›î¿âQ–?òß0¿îÛK_ú¼t?çGÍ+¿ìÚǗæd¿ïÿå"m/®UNASNone?î¹³"ŠL'?¤ÖtQ?‰VDôëh³?öêò@"ˆ?œy9h0µ?›ep'¢m?ïÛÇ9m'ˆ?u-ì!#Ú±?DNÐhB?Vy'ËƨÌ?o%NXH?qk;kõŸ9?íìþƒÜ¡Š?Ÿa'H†Ú?xâŸûS5?€'ò?®×»?žneF'm?ïêF ?R"×­]ì#?Hÿ
Âê¶n?ABT6²K?_~VP#më?N—ÊKI°W?î<ô5­?¯yƀÝ?"ë'ÛÛa?ªÄø´Z…Ë?¡»(·8£Ñ?¡,—'{
†?ï"/Ìôí?•˜ÕšO?Yb\<Ö?£'ŠÃ?‹Óà#oà?''MÓo¹?ìÜ4±(¤?£±kQŋ?€ŒÚÈ{Âä?'ÌYØ·?·ÃÐj_F?£}§Þq^?ﰆº2°?yŠ¦ª€Éø?nµ}²<ü?ròêBM]?xaäTàxl?ocŽŸ%,AGN4FGL J1258.5-3406¿ïÅúÜ»¾n@<¾š,fXÀ:¥{ 1ίÀ<U /Äê@Æs—Qj×@@D
û?ÅÆ÷ܔ@?£uÌàÃÏ£?Ü0«½@>älP¶¿çž¬ÞšÕ"¿ã¯=šÀ5¿å>#¶e¿Ûa®[G¤Y¿ïúûHáb?ïNž=î"2UNASNone?ïe!ì3³?…â®+9#>?däa8‰S?YŸFNêY?¿6Vì/p?"H$c7	
?ïD,;?†³`–àÛ?cbŒl«i?i »…ÖYñ?…~aJ·?'L©ß,?ï12–;|i?ˆôfÆgì?sêTiÞæ?u¸+Œjü?"ß#ÄGœ?"14AÜ\w?ïoóÈd2?q(*0Í¿?dbÀˆ&šÁ?MþnÿÒn?"ÒáænÇ?o;¦g9øX?î|Ê%Ü?œÞB2X˜?y&ŒAþc?pù'ïW?¥®Œ‡ò¯?›V"È_¼?î÷¿ó±¤9?œ¼÷[…{™?qQíV±ÇÌ?}Lѱb_?œ³†:þ>ñ?˜Ý
Œ°}?î/<š©Ó½?—üaRò?-Ót¯?{@삕^0?¨Àî¤ç?:?"¡('uÓ¦?îöµA?'Àh«
?€]1ÝëQ¡?plë{¼¡u?ªÉQÜÛQ?'NŠŠY¡AGN4FGL J1259.0-8148¿«ò$üâßÌÀ2òã'÷ÓÀ:4·b|ØÀ;úÏ®ÿ\l@U-ß6[Ý@1Ze§#Æ?ÄETÈÚ#ø?Ö ÛâêE"@:¤vlmç?ù­q:)òm?ÌÆQ)³¿à*_"ÊÕ|¿ãnO3Cú+¿é°¥ŸaY·¿ïýá!˜¿ímî$nUNASNone3FGL J1259.3-8151?à«Oµ¨?ÀD{9Ýz?ÄY"6œÛT?¶R·1)ú˜?Õ¨´'?¾ô€§ÒŽÐ?æÀŒô*ðÖ?ÄÍ^ §Þ^?Éhùf'b?Áª"Ò.¶?·)¥"=ƒ?±¯J¥?à÷t,ïï‰?³P)®½'?È1é$Nò_?ªÅ["í>'?Ñø#åÇ?°œ}[—Í´?ß8ìMÏi?¢
Қú?Ê*o÷´­?GqŸ"Ç5?Ó±ÓûGçÿ? »–8yÏ?Òü"õüØ?½CU÷ûœ?ÌÙ=ò1"Ô?¼¯'̘@ö?ޖÍê^?Â@p¢CP&?Ü«G˜8¾?Ìe¬IS?Ùµ%v\'É?ÌʆZ'_Ó?Ã?&Ø>ò?¹<­°¿à\?צ»c™?³Pý¯;îù?Ñq´Ö¿rz?³â×Ëބ?Öè<n4)í?³''Ýf?Í"ê+¾…ó?¡áÎÆßéX?ÒòÞؼL?«îw‡ïú¯?Þ{¬º?«‡`\C«MIXED4FGL J1303.1-4714¿îêaÑ3íK@/,e@ÌxêÀ;$zØä2DÀ<×ïÖ½—@?$š"v?ü)tˆhî?ÓÅá @è(?çruÓÁ³"@l¨ýº«b?ôÿVø4Y¤?î¬âžž?àdÀÿß¿ÜGüN¿Õ,HÓ
¿í߯Þ)–|¿ïü2JÕç(UNASNone?×màÓ¿Û"?ŚZòóZ´?àëþ±{?ÇVÅ+?À¸Ž^IƒÏ?µªåâÁ'v?ÉÉc8÷?ŗ'°¾œ?䔁õÁ–@?ÈHG¢+
 ?Ãä"ðùŽ?»"CP%¡?ÞÌñÈ)?³– f5•Ã?Ö×è¿qšw?³lŒ÷…ï)?ĶLqŒy?©}ÁK	IÈ?Õ!þÕ*
ã?­÷zb0j?༘[Dãù?³»AÞ<xç?ÂÉ è˜ZT? ÁáÜÈ?ÖØÍI|ÿ8?Ã}¥â¨+?ß|ŸksI+?ÆK`Vœ?ÃU&˜E0·?¸tÄô¢e?¹‰¹køÊÍ?½ŒÉÂ|o?çf»r®k?Ƚ3æcª?Å 6ÌoÚ®?Áë_£ÃWó?×Õ$B225?¶=S%·Œ®?Ü ¸âŠ#Z?¸í‡+¤?ÈE¸­_?¯û¬TÏh?Ä"D\•?©Û[þ%ã?ãÇÌ'ãt?¼b	`ë—?̾‹&ËW?³R0¿ß€MIXED4FGL J1304.6+0539¿åA—P$kÖ@QÂÀð À:çï¦ìhÀ<"®‹ÜB@£ÒW%V?þˆ×ªva?Շ-;!"$?àžÑç¾Á@}!"Î~@·ü—•³[¿ícƒ'ǁ¿¯^L€PJ¿Ûö î¿æ>$}㰔¿îxùæáK	¿ìšäó4?£UNASNone?îëB=è?¬o)#Qù#?x…œ%&ãi?sö]$H?œvQ>V¿å?¬#‰&lÂ?î̕;úO?ž'Ðxd&?Š®cÉðš?'u…«4¨}?™,«ôSé?'ǺáŠ@ƒ?îf'4õ?˜.pŒÍ0ß?—tñ¯à?Yõâ.?¢È3çñ¾?'`Lo:¦?íkƒ™R?‹`þŽ	d?˜"ÖûÊ?€ŒÚo}á_?©Ð)ô?ƒNÇ=2¼É?íuÊê@ó]?¨¾9 °p=?'•:¥|á?Š÷kÁ?¯Ø´ֈË?¥Ó¦TÔ?ìÇ P ?µIãZÐ'˜? Û¡÷˜À?§îY\º+?±Y,…pÍ?¬Äß1m$?ëÉ⡗·9?¦ZSë:'?¥ñ'Ëá?•¨Žjk¢ž?¶¸)âÞyK?¡å?qp_Ø?꫙Œa*p?£$åÌ#äÊ?¦"÷gbâ9?•*'S›ª?¿X·çmf? "mpÏS˜AGN4FGL J1306.3-6043¿ïþ6¿ã7ü@ÊصýÀ8kÚÜZ	À;"KâC@•û¯
t2?ü瀭9Š?±=z	3?ÝXʜpäo@)ð$p!Ñ@ú F˜7¿Á"Ê|æZ'¿¬\w`o聿Â1ÅIö™$¿ÝM1a!.¿êŸwßµ‡·¿î»úýŒ³,UNASNone3FGL J1306.4-6043?€×|_îC?'»ôÍóă?íÓå`J =?²¼Yô3H?®¼ôs¤?±|ïªGfÇ?‡÷ã+'ö?œ¿1çUO˜?èpá?Áƒ#~'à ?ÌÀIÝ2?Á³®
óV­?ÀÐmœ¡Çø?©jÜ¢Ù?çéøÿ8b?°FpNÊýå?¿œþ¬ý?¦¥'Äíø?"ÐNð$¬?~ö(ç
?çê=ÌûW
?¨ە<'­?ÍÜþí ×?¦Úw1~—?€s]ÐT¾Œ?ð9#:?î"}6GÌ?ªÜjÌíý÷?ªyà¼yàš?¨	0?Þ¹?|U"‹ÔUË?—®"Q!Êo?èÂÅãà Ð?Æݑomd÷?Ì<K=s²?ƚ}w؇I?²HdK°·Ö?¦Š'9?éïàŸV`Ï?±-åƌÐ?¾8–½yÑ0?¦ü0ãXǛ?võ‹›ËÁ>?e%?6mª?ç›'ü`þ?°ˆ­	Ï<?ÐmÛ³£
¿?¯²J:»PSR4FGL J1308.7+0347?ígŸSgC@P'˜ÜÛ7ÊÀ:¤''%ߎÀ<1ìVu@t1ñê"?üÞ£©½Ô?Ð*¤CkºŽ?×ØJ"]?@_"YÒÚ@k‡ÞY[?îT  ô×®¿·]
½ô¿Ê˜\©#O¿ããBZ£‹¿ì™ V¸¿¼¸ÈúÃUNASNone3FGL J1309.0+0347?îK£I›ªk?ª"ú¬¿¯?ˆãBÏ?Š_°I­?¥BÊ,˜ì?¥&´Ö?îåÙ[%•'?žOc°ø‡›?‡¯r@[²%?'}6ÿžñ?—m|×BÒ?'Ñ}•ë?íŽ&¦ÝÏÔ?Ÿñ2B?NÅØ3T¹?'R•ºl?¨v2©xôX?–ݍr‡?íù¶«´_?†Êlƒ2?Ç6󢝦?~÷ðǗ?¡€ùÉ0ëB?|e­ªóÀ?ìÀÈ´±šd?¯êT)õ]??˜#W%´M-?'=UV€?³ðä't
?«hµa{d?í/lÁÕ"?²¸‹?pQW+¾?¦"Yj¥Fh?®Q…þÿ?¦ˆÑ±È?ë6vuÁçÛ?¨ï=Ù c?©ðw óÀ'?™Uì·
1?¹TÂRÇä?£ªÀq?up?ëÞ ¿}®×?€/*Þý†?§q½¢+qD?'s0èïÜá?µR4´ž ?–:вö¼ÿAGN4FGL J1308.9-5730¿ë7`;K|ø@&ôàM/À:Ž 'F¿À<{æ*kä@—"§Šs?ÿü€ï~¨?Õ)ôzæ¦?Üxù!¶3@¨–2æ@¥¿p÷z? JAòh¾?ì¥~tz%`?Ö­Ò HÊÊ¿ãw?}ÄQ¿çæ!‡+¿ïÿž±0UNASNone3FGL J1308.7-5738?ékï÷Áy?¶Ž‡ñG'?œ±û=¸??"Ô£…Ö™)?ƺ·Šñ5?´Ãt	?åOÕ?ÃËðò?7ïþæô?ŸÉ"Qâõ?ÓLq%dÇ?Áî$ý ¸Ã?êtjÇ7ü?©~)l.(<?©âáv??™€_–%ŒP?¿ÓS98ÿ?¤.ˆ©‡Mg?éÂYyÌ}O?¡­ø¦
? $eÍ?ƒÀ‹'3Á?Äí–}Ò¶? ·ËF°€ ?â_'Âdéå?ÀÌ1Ô/äì?²WrYf?¨}ùŽ£{®?Ö«ß=Æ=?¿A
G'Í?ܕ+­¥6¨?Éfƒ*ø?¨"áʏú—?¯ä0J-r??à,,³?ÇÓö×ã+^?å"ÈP€ó?±¼O^Ë?´¾Û¶Ì9½?¢Ô~96›?Њ¸q1VË?®[ž9?å…Ûv³¼?±4‡Nµ½?£ÙÄ-Ì)?"C}
ö0Ò?Óo™ÃØÄ?±+ðz79äMIXED4FGL J1309.1-6223¿ïÈAo.?Ùõ7d›5%À8âŽÕñÀ:é@oUxW€@ÃWEa3!?Àø:8àò?ÚzÁÈó@ÔÌ?ß ?öˆÇͱտïô;pïVe?ïì´É Èb¿âÀrM'À¿êÍ»à~í¿ë'jxÅ¿ïÿ÷Ò4ÛUNASNone2FGL J1309.6-6230c?´-í¾¨Õs?Áq¢é•?æŽÅ —5w?Ëǵm¬ù?Ë­ôž¼²è?Çñ…à÷?"ÍZ"­?ŸûI¶")?׸'´üT-?ŧv¢¯Óÿ?ã…LT¹¸?ÅH/üiió?»'—ëæåÊ?¨w¨4qÐ?ړ÷œaӍ?¶ß›è§2?Þ¢"i·S¿?¶™+ o?qß{I¦'ú?Vb'63C?ÔxØGÃýµ?®MÀ¼Ã÷?åŸÔå±0u?­øl^î?¨ƒZà2?ÅÍDiL±?é[B…Oy?Ë&£io5?Är1ÔAø?Ãé.•>G?€MNÅÃ?‹`ééÓ?Ü3ôËæÀ5?̝MÌDD[?á¤Ñ@Øjî?Ì]öºJØÛ?±¶p{v›?¢@
DŽ8‰?ÝÂåe[5?»{¼¤º¾?ÝÐK–Ùå?ºS9Û:p6?KášP[x?91K™x?Ú'{"…¶8?¸ÄJÅ+?âåQU)Ÿƒ?¸ÁÂ:‰9MIXED4FGL J1309.3+8035¿ì÷Ø#à@BALD|0ÓÀ;*qgKiÀ<xÓâjÃÃ@y7OË@ÖÕ"õÎ?À°àÝûÉ:¿º÷Tføˆ?ú.Æݟƒ?÷Od¤šS©¿ËÊõQÓ²¿â¥ôñ¯e¿ì˜¦ŠB䁿ćœDCÒ¿ë†lËÛ5E¿ïÿ••_xUNASNone?îÂ`ò"
±?²²
ž &?ub¡0C?'wÇ´úf?¡-œ¹gGë?±®öñ€?îõào
^? C<§¼w3?ˆ.Ã\•ë?"Yô%çi?•,iµŸ`?î_×q'?íå9 é!Ë?ŸÅ;@¬?Ž_ï@úwÿ?Œ\Ç&?ªj$žáP?œTh–Û?î<òù‡@?…Oc)?ö?"ÈÌəD?hN{>¶Þ?¢[jÄJña?‡Awž»û?îÊ%cÍì?¯<»õÄZ?–°€òËè?ŽLæèbó?§M±Œ#D?¬)ÇAP5?íÍÍ (Ì?¹ÁÌœÕ?¡ïÍñ¤˜\?²À-'ko=?­#U0
Wå?¦¤Š&´?ìý…oý$??¤‰-wȾ"?–S›?'øCšŸÙ?²'¿˜	`L?¢;Që©2ž?éŽÀ†1?¯¹a釡'?µ™'zd¢?¨ºùÏZî?½õÑl³vS?¦=²¤=ÉAGN4FGL J1312.3-6257¿êÚ²@âüÿÇÍùóv"ÂÀ8š"O…yQÀ:YÔQüL@ (~oÈ@¡Tÿ5Õ¥?Á÷ZjÔÌ?Šƒç€­:@I=Ùb·@C›`C¿ícþ¬Bê?ï(SÜ '¿á"æ".¿æS®h]·k¿çqß
¼òd¿ïü"à՘MUNASNone?ÃI‡LSÚ?µÂñ¨_–O?¢4~ˆ4ì?¢uÞÖôõ´?ê%½m£
?¹#jº–]?»§¾uq?¼?5†/ë'?¤à :dÙ?¢¦O»ëX?ëP‰í?½úæÈmä×?ȾýJù?­¾yŒí"?ÂKyn3—æ?­v™Ò^
%?å=¡%ª¨?³§vĝøP?ˤìúÐÒQ?£€šÐÒr?¨ó¼Ú@ž?…Àç|«–)?燈ó·¥Ò?¤'€n·f?º"ÝF[rÜ?°z<ýSR?¤Ø\:"ª?£ë+»"^?ë_þ"vóZ?´¶"^íš?³]»þxŠc?±¯+á/?®Vu)²?³+aeBƒ?ë®çn¹œ?º»Þ#G"?Åþ"DQ$?®œDCÑ»õ?ÃG¤9/Ìv?°û†]L˜Q?å®w
lhù?µý€Oâë?¶V.‹™?˜íÇ3ÔÅt?°_é%œ<y?"f­rº=Æ?ë)=qþÿ? Íþ¶_ë&OTHER4FGL J1312.6-6231c¿é´÷UXïR?Ï!ٙŽÜÒÀ9QTsõ›"À:\Ä"Úœ@±öÃkO.@üØ:¿¯?Ґ`
à?Ü;\L‡@±žs.?üYçՑÂ`?åk¢E9Åô¿âŸ=ÙFX¿â1e"n"Þ¿âÓiÔ¯ð¿ë‰â!GÎK¿ì5?|í'UNASNone3FGL J1311.8-6230 ?vƒ<K¯…?|†ý
F	†?À2°b{#?'ÿLȝ£?ïL÷òaÔ(?•ï".Ê?µ˜§'Šô"?¸¶£¬_Gx?¬+˜§Yµ?ª~֜DÊ?ë"Tð'?»_Äv<f?¢"¼_8Â?ª¶ŽÉ'@ö?Á~M¥Ð?¨2¯QУ?æ÷Þ½~êÛ?°Qᕣï?šâIþÕL?…LÕÏF?¡[€OãÆx?Š•wLÇì¯?î5«Ù&?•ÔÜ]/þB?rxŸ?øà?o™™Œ‹¬?•˜'·P¥?ši Ü®Ô?ï.MƒŸ?vÃç?¢_"^‡¨?§èmt#à?®ý¯ØE2?°-µ÷.†a?ìê+ÂHö?´ð'Ÿç?µ[wC/4?œ{æÏY#p?Á1–X¥N?©§—}ófc?é+^Ì?­²"gäá?4·p-àD?pÜÈ	ýŠ?ŸíUú'J?·õïÄi?îÂ+äèÕõ?"<ññ÷OTHER4FGL J1315.9-6243¿á'g^D??Œ¥šŒf]áÀ8rãËìÒýÀ9ãûó+g@Øçk´"@jZíŽ?ÃÌMß?;I§hå@ýœ¨?ãG_ºü?ämªþE띿§Ãހm<ˆ¿åwu³
"¿èœX@2õ÷¿ìPޓɡ¿æR£`—ÅYUNASNone1FGL J1315.0-6235c?ÁŒ#+¾?Åkô~Y?à̜Œy\?Òœ²ã9?×Ud.(?Ðöf?ž–Œ!u–f?¨˜òßò?ÈX'&^ ?¿xN§¶p?èõ+€U?¾ýÈ5kû.?µi£[¯?¢emo©?Ñ׍'ß?´þ¤6/ÛÉ?ägߒ¼?µŠã*‹?fÏJ2'£ÿ?L&
wʾô?ÇË$	/æ?¢Šæ8ÐÀ?éöi¬þš?¢™$pü<?°†Ndò0?¾¸«ú牴?áq"¹W=î?ÑYÁ#ka?Ù˜ùœÊ¸?ЪêJCY?‹Ôöù?–=ïx$/?ÊkȐ}L?ÃÖJ'Áþ?èøõÓ½h?Ãwú<ª?¯V›ûÆ ?šã'#B>-?Õ4Frn÷?·nS4çZ›?ãŒrÐc?·F6š®²ÿ?B™4ÏJº¶?1æâٛÀ¥?ÎSFùä‡ÿ?­éY¸i?èf‡ôU§Ò?­ëðãß6RMIXED4FGL J1317.5-0153¿Û to²_@N&ìAÝ"À;DDfa]éÀ<ø0À'+ç@"¶'MÊä@Ôxã@¬˜?ÑùcCFPÇ?éizi~@}¯li¶?óQ½ØP:¿ïÿûÞ]Bü?ïÿØBKÔë¿ÐgbdÏ
¿é[O6Ÿ¿í"}¶98¿ïö¼?5õÛUNASNone?Å6SÀÉj?Å8—¥gqî?èXV¶E ñ?ÉÐq`Ú$?²Ð¢Ï@?¸šºmœ*?º=™0Ƥó?½¾y?H?êk{c#?ÁmCԄëÑ?²f‹·D)š?¬3ÍÀpP©?Ø [x€?³Z;egÖ?Û¨°a…ù?´GbÉ¥M?ÇneA?«¬'_®JÝ?³}'ÊúY?"j\ܵW?ìfôa«?žmg/»º?¢¤4jO[?"/`­Ï8?À:¦»Ÿ?¾}–?Z‰?èŪ>-?Ç%ÎVöÂü?¹cǽ¨Éa?½Ì.c¸³?©ú¾èØ?µ¼~G™ø?ì4G
ç Ê?¿ùïb×nD?±`¿šã…F?°ƒ+oä/?Ðá.l¹q?³Ä¶‰Ü'?áI×é¥9z?¹§4M>Á?ÉCƒh´?¯°Ë)'¤[?T£/v¢?yÊ•Øo?îEÃ+
tÞ?š}3)œ9?£y{¸z]Ô?˜tøÄZ4PSR4FGL J1317.5-6316¿Û<Jwâ)¿áÄ* vmÀ8àÛÿo·HÀ;Ài;'@ÄØâ"Å@Ac?ÁÌm‰gÈ?â›êÂ+35@XÞô½²@Ì$'óÕ¿Ò¾0×@¿Ð¯ª}¬¿ËÈ©¼ýKñ¿æӉX=¿î<ƒß1i¿èPž¨øUNASNone3FGL J1317.6-6315?z´¢<ã²?{UL™šA?뚢:B?½Ldz!Cá?À¿Ò¤bS?¼VËӘ?uuÇîÅ?¡d¼8ž?àÍB 9ö?ß:3Fm?܎$–ˆ?ÃiNåsë?¦5Qtօw?—Î>IJG?çbàÕÝ
?²Yyë?Ìç(M|	¼?°ÅùÏiä?¥eû˪ó?l£'ÉýI?חlI:—½?¦<ªóa ª?âÝø»Š|"?¦Ì"ì‰Ã?z^ôá?rÿ—†	;?ëŸt–n°§?¹=I§1ë\?À¯=@Žv·?¸mð"¦e…?…áŒÇ¢?ŒQ:7çÖq?àÜçû¸ƒÑ?ÊÄV[¬N?ݗ't
C
?Éô˜|Á¥?™œ°×ØQ?ŒB¹'pP+?è5ùW€€ª?µt6hæ?Ëô"Ÿ•Î?³ä'O‹=?†¾_/,K?hW	Ø@%d?Ù7ïnüü¯?±²ƒ‡}?ã	ÌC‡?±¼¸1f'ÈMIXED4FGL J1318.1-3937?éÕw÷f"@6óNÒöÀ:O!Kª"~À;ø>ü•u@¹:"úžA@¡{j×?ÀR‹vÁ¿ºº¢Óª?ô&Ã$º@ϊxis6¿è€zC'üÇ¿çC{[¿å­Á±ç¿éEP6y8Ñ¿ïþ3ý]ŽQ?ïöW_¸LbUNASNone?ï«yÁôñ?Œ¶ü
dù?}ȹߋž‹?ˆ¶bó­EÐ?hôÊaå?pi짎qï?亂Ñ_â?ˆµPz
Ó?d½÷Á¬Ÿ?sf!<7?©ÞGš?0?sÂtK?îà¹e3X?'{èúB
m?w^±–±v÷?yîª'li?ž'üsX'=?ïê‹Å¡?ï©lû"m
?i>¼é&âÿ?[†™¤»½"?IïȐm×?'3î"—Ì?f˜9!%Á?ï0ù-d"? ‹îtãò?•h¦ð‰?ƒý°Wf½?zÅ@±^þÜ?‡Íqª•©ñ?îÿÔ0:Ò±? Ov…¤aw?v»T^¹å8?‡1g¦äM ?šV¤ãŠåˆ?™Í¹|èþ?í¢½áÓo?Ÿþô^®ƒƒ?Œ8Ã›Æ|?‰öÌ»à	?®Åý¿w¾l?›"pØïÁ?î¼Åbl©?Í÷k°Ñ?{$·så?rÁ}ð8? Ó‡öv?‹ŸÌ\¼"îAGN4FGL J1318.3-1148?åÐ+›±™7@IBA¢a¿8À;8P©fÀ<þº…¢l@ °u±²ë?üÊØÞ¨—?ÌjØó!?¾úš ¹D@?õyç='@QŒõœNÖ?îåÑ0é­?ëEÅ.î*?´OÝà6r¿ç˜S~,Uɿ̙%•æ±¥¿Î•#éTqUNASNone?ï¥'Õ1?z§µ«¶?F'Â~"'?>Ú^ùmQ?…XmvÈU¼?yš¡rL?ïÈ
	2¢?v@ê_;›(?Ln9%è³?TڜIÉa?xm4OT´]?r¸Ýƒµ ñ?ïFÁ|PwV?ƒ¯´0œFœ?`¾ž¼';â?W‹Aù‡Þa?•ü¤
HÊ?ƒÉ"^¤?ïJ'mÞÞP?v›‰ ŠŸ
?eòîA` h?U"¨F½í?"ïTÏ‡ï?u@Õ¯]Éß?ï<¬'Ë?‰î)£C?[U"æ2N?P1ÑM¤?–µ‡6ü¨?ˆz	 Ža?ï`ËDÙ¤?5xxZÜ?]‰Ï<_Í?gÀ¡Ç˜¶í?'
ó×<¼?iÂŒÖý?îX$¯6å?'BñÓR´?ll+ã5×l?iY'I×È?¥3ºø¦ÿ»?\½¬Y¡?î/9\Ä?"Ý=å1ï?sí¾ç^Vù?l"f.r+.?«ïTŒúBß?"WÕHHAGN4FGL J1318.5-6352¿Ø®J«¿ò¸LH
À9ÿxǑúiÀ;
–}…fÝ@!1{{vn?ÿ܆铬ñ?Ò‡B)V?È'SV\ÿ?ñõ¿Ÿ½ 	?øVª0À'¿ês.0D?èRÔ¨ù¿êę!¥¿âŒ aßÄ¿à¢*aÓY¯¿ä²@¯rŸUNASNone?¾t}!á´?·‡ÿ
F0å?qqº›¨+?oœV²q0_?ìŽN?†±?·Ïיœƒ5?ɘ¶ÖÒp?Ãƽ¡;?–Û^(
û?š€Ýµþ);?é>áoϤ?ö¶Pð™—?Ö¤XRÁ?²Ï#¤âÝ?¦½áü?—¦úÔg¸Û?ãB&>
Û.?²êV¡Q'Ò?ÎÃxM¢'æ?¤é³öèá?•m–ý]
? ö'ëk?磹§šÒî?¥ÐLJ'Y¦?µ²fÙÞ?­lâ–ŸÏ?y‰åì‹]‡?t€žsSÐ?í¬'Cnr?®U'5ÌV
?¶¦Ç-}F?¶*¼ÒkS?• sÄÇŒ?¢ÞB'?ì'#|¡â?·ºtwτ?ÉJšÊú˜?ªrOèE…8?¬‡C¯ý?ššß8½Ü?çìCe'Š?¬ÂW•š0?·òE†Æ!?U§+œt?"(¡nV9?‡2
g'³3?ì`rCòÑ¢? …~dÌí¶OTHER4FGL J1318.9-4556?ïö*qe@0¨àP7PÀ:kÒPšLGÀ;ɯe³¹@ëÙá³8Ò@
•Ât"6?×n†›e!¿ æÏ#á~?×ÝلÁg@Õ(eú±?ï==B€®¿è;/`Àµ¿êD~d^¿âÔãâh'¿á,Ãã?l¿ïÿùµc#¼UNASNone?ïVˆYD-Æ?þ/¦}?q"¦T®Ô!?rÒMjš?ÊHÕÔ*?‰ß‹±È'3?îñïHD3Ù?Ÿðî1yß:?x¾</?|£,¾ò"?›½gqVÄ?S±þ¡Mq?ìkÏ1‰˜x?¥0¬^,?—p@‰t?'^Îxó?¶Åf#þëa?¢B"¡V²?î%K·Ïæ?‡É¿O7€?xFÆ°¢x|?^öóªþ3?ª¢vѲS"?†VúýP'?îÅ5Xù?žxþ†'²ž?'r÷R!?"hG/0?ž&=¸dŽ_?›"TA4x?í"y{hà?³l[øî ¬?Š®"Ù	¼?šißՃ£»?°†o§·ýM?°ÌÂç ×‰?é¸B«KH?­¬bk|r9?¦ò°*7ˆ™?š•¨$J-?ÃaVéé	¼?©ð?G‹	?ê'Êêì¿Ô?£a‰"Ú@g?"%Zy—G?€‡Æz¶?ÃT0ˆ!æÉ?¢_1Ë¡uþAGN4FGL J1320.3-6410c¿Í'w'¹4¿÷£ÄzÀ:ћh¦³À;cp£×
=@V%üi@·—Ù¥ù#?ÒO/¾¹¸?ãšb‹»`@ãI{t¥@žtGP?¼¤Eoóe¿Ø®ÿÿdû¿ÝSV>PοèöуòÖ¿ïÿý¡UûŠ?ïçÚÄç%UNASNone,?ΝI-ÐF?½ãÅL2*?À$iÕm_?¹cà7(Y?äO"?|0—?EhÈt?Þô³Î?ÇxUW±}ø?ŸvǺ.e?žßü´®äS?ß'ÜO»n?ƀöë.a½?ە~#hÝ1?³+锍þ÷?»OÊp0{?¢q¸[?ݖW»±?³X{ëÁ+?á™ìˆ?°v8ö©†?ª~ U0Å+?‡°nË[é?Ù}þ&×Z?°4›I9]X?¸ ËřZb?®&)²"?Çë ÚM
l?Á×k£ße"?çþP¹'?ÃeÃä´?Å՞Ô'EO?À6«©¢·a?¥ÈÅè=QÖ?¨S
19ç`?é.ìrY?ÁDWhÈ3?Ëp(Yîç\?¯vA+œ4?¾§åŒ·3?¥ÌÇ2Gê"?åNù7í_È?³C÷v{?͔QjD±$?­ë酅´Œ?´(%¡ÅÐ?š›
5hYÀ?ææðÿõ?±w1×ìÐMIXED4FGL J1321.1-6239?Ÿ&Ï6Yd?oÒÃ(U¬À9F&yçL«À:=­P/Ã<@Cïò@Ï©@›çl‹C–?ÇmÍbôÁÞ?Ò7Ý ×ç@¼4 ˜ü¼?ÿ|ºñXw¿êö$Û?ﳨ~cÞ!¿äOÒ`_'5¿æ?_´Æq¿ì†väÝ¿ïÙ2ÁsR]UNASNone?":*ÁE?Z?€3òxˆP?šJï 2ü1?£~'"2>¦?îÜ¿Øò	?¤ˆµ"‹Ÿ?¼Bå˜m?¹‹Ž=?³Ôô…ð½?¬ˆ(µg?éú='ŽÛ?ººÛÍÿ¨?¼b µÆåœ?¢~1ðNBi?¾^ïà´F?¦Qo3iŽå?è§Ýì§*?¬p"ÒO?¬Ô׺ú²?•¥KÄó'<?©º§ÐüÍÀ?`úÙ´îˆ?ì—"û©? ?ÏÚ»{U?$]©'®Ã?z¸sqK¦?›z?£äFæï7Ü?îâ¯hY?¥u0¸/?¦`›g£H?¦ž=â÷w?¸9­Ô¯²D?¶ÇÚÑ/N?ë'À&Î÷?¸®¼K?±…é7;«?"%ã`ÚWÇ?½V:ÅßÙÖ?¦ô.DÛ/?ê$†êaÕ?©›>•6?"†:£1Kf?…²Ê"œ?®efEW™?ßÛpŸ<€?íu|ä' +?¢oª»]—=OTHER4FGL J1322.0-4624?ëoP¿Nù§@0!y[5°¼À;¦v îÀ<ah#ÕÈ@õÃêûáã@ÿ$7í­?×Äzb?áƁŠY5@ÒõU'"@†Ùû3'¿ïö!Ÿ·ë¿¿èJ ˆK>?ïúÕÔ&]¿àwÍaGBµ¿èÝêa2Iÿ¿âG롤*UNASNone?ïÔ{ÿ?.«}áq
?ƒ°Ï½®Q?{­*ÜQÃû?'-56ó¦?†ïþ×¢C?îíç\£¢?œÔ©Êp$v?ƒÂá5Â^$?‡£¿èVÎÀ?˜a£ÊO8?•^»§Tzþ?î_ԕ²É?œL9£ŒÌ?ˆ}ÛWg
Ÿ?"«ë«sÜ?©Z‹å"Â?™)+)?íúzV?"ÉÏ(¥Ù?ˆ+[ ܸ?w	#B¹ÞÀ?´jÀÉKrv?"c¾k` Q?í-'›x—?©^cvg¨j?Ÿpy˜Oö?—oIu%,F?­wJ
 {‡?£iý`ó¸?íF‰Ñœã?²_&b1¦Ö?™ÕûÞâL?¤Y2&fó´?®³™Ù‡$µ?ªZM1ï¸Ë?ë髶fö?¦´¯Ï¯ãÚ?•ú(C£ÀO?ŽÜC¡æ%V?»4>ñA?¤"jd÷?é}\eöC?®¢ùF€×|?"úÃTJ|?5öíë?É.Èõý¥?­²Ô{§GAGN4FGL J1325.3-5413?ïò³L"N?@ ž2~ØM4À9Д®xMïÀ;nS™Û@ŸOúi=0@¨˒:*?ÀQii¦î?Ð!û'©@ëÇ~¯2ˆ@1õ桊)?âìv Æ3«¿ÍMõVXÒ)¿ä=1NV¥(¿æ´äv]¿î^? ÿ¿h¿ïùÁ­UNASNone3FGL J1325.2-5411?ÓV…ýI[-?Â}œìgûE?¶G
Öcl?¹
§ ÆÉ"?ã'ÔÉÁL?ÃÎ
7o
­?å]¸ˆOÍÑ?ÖՆ§?±ÑúNŽy?§ô¨¥«?ÐÐHðè=Ÿ?ÁT,–ЫB?äñb."ˆ÷?±Á@í$?µ•ÎôD`? 'ÔDÕ?зÇååÖ?¯ßéÚÛ ~?åg&=]?¥Tc'ÄIƒ?±òOóL©?Š:iI
?е°»?£ó%¡>Š?Àf¸øNl?³æJîï?˯*ûVM?¹ú¹¼q,_?çfÃÒ?À!õéP¼?Úý6"ÿâ,?Ɋû†ž•,?Á#ua<A5?º]HkºÊR?ÜqÊaý:?ÈÖӋػÃ?Ùb{å]?´{n}ýõ?ĖáÒÝ ò?«*Õ9½?ÜRs™™ˆl?³¦éY› ?ڍª&sv?°Ç\Á7?À«9-Œï×?¡M@7!?ݹA³1N?²˜ÁÈmß°MIXED4FGL J1326.0+3507?éÊ`!'Ã@SǘJAÀ:à=ûäÀ<Ð;êŠM@BúÑlð@¯_ü¿ÙŸ?ÄR†J1|z?À
W¬dM?ûL'"Ғß@!ü@­Å?ï4ãlK'µ?«5〇=»¿áËË]k¿á×>–¾ž¿ãúQjUß0¿ïýí5øàQUNASNone?ïÓÛkÃiï?©0Ar?R+¢VgÑÝ?"=‡!(c?q‡aŒ °?¤MwH4B?ïâ"ö`U<?mþ*¢ã<?=*qø{¶?H2öbRNl?j<ä€&dÆ?j
¹@H[?ï¸jóš?táŽËîT)?SÄÉÅ;u?S&•.:¦ö?~Ù¤W8"?s Âí¢È©?ïä?ÒþÀ?K`Òbü?U L±t"Ê?:²F…‹íò?`ð§%Ö¤?FQ6cù\?ïÑŸiè?@-Ö!ì?Y4{8?pÞpÇ<î?q2×úBÕ?ˆ³Áuò¸?ï R'è?†€áß%u?P5bôŽ½Æ?\©'@Õ?…äÌ»'?…Ì:·©?ï~'¢Ì•'?súºý¹?]¢`ôR1?[+¯¸jAI?Œ§K9ãqA?€Ýoåq°†?ï²å=Ì?hŠg3¼?kWÛzaàc?WîÞ7ŠÞ?xás»¢!º?d‰'ÓAGN4FGL J1328.4-6231?辝 [Í?§Ë@ےbÀ8ÎÍÐØËÀ:d3çüÔ@9´ú,V@ü``'çÏ?ÌŞÛô2?߃>ÄE@|h½X»ƒ?ô#Ãy<
?ï°iS?Ã~.Ú²¿ì!-Aª¿ëÕÕßðëæ¿ïu'Þ—$Ÿ¿ïÈzη3UNASNone?À¶Ï~?ÃÄY1…Å8?ºÑÊ@¼?Ä¢¸¼Ÿƒ?èxA|
©?ÎsàîÌ?¼ v±Ñã|?Á+þ<ÂË?Ó(Ja¶?ú÷ðˆ‡?âç̵?ÅH'mú{Ô?ȼÏ/8ãÝ?®s÷&EA±?ÁÏï
‹Ñ&?ªçª0±î?å\ÐpÎÒ¿?´F#­õ•E?—òË$†;&?v''ÍôE\?Ù5;'À°¬?±@—Jº|?â¥Ì$±!?±œŸ<ٕ¬?µ4qxr•d?½óGÓB!?Ã.Ÿ˜¿²'?É2+Ì6¥?èÉêøºo?Ðnt7	‰?Ÿ8vF¶ÑA?¨›¦¡*aÇ?Ôÿ*kþ»?ÉÍ_S+Ã?䆧Ë<™?Éy«ÿM¨?ÂÏÁ«¨Ý&?«%م!Ow?ÁõÑäõɬ?¬JPÇrä²?æΛØVK?´^(R78?xw½‡Ò 5?`™~B-}Ž?Üη3ĎÌ?¹¨hYÿ§?ág´ê­ÞJ?¹Oe˜áOTHER4FGL J1329.9-6108?îsˆ7¿?ö&Ks›ÙÀ9œ§ktÀ;^iŸÖÊ}@Ù؅½™©?ÿà,%!øx?½ø+஁?ÙÒüÇf[@710ýÏ@®€™B†¸?í½ÚÁ'ï¿Õ™0þz™Ï¿Ó¥!ÂÈg¿ã¿YG¿í-¢Ðzw¿è@<›'Á^UNASNone3FGL J1329.8-6109?£Sb}£š? ãY[Yûœ?é̾bâßo?ÁJHbý·?ıœçú?½šëSJ«?µ‰öBaÛZ?Àk¼ð?Üí̉ߣ?ȒYج2?ݯ¶S0 &?È·¹6ºI?¼?•'nŸ?¦£ˁô?å"0‰z#?²ŠÀ(à°?ËϸO`%?°
vKþ߃?ʾð|e'?Ÿb`€?ÖÍѕŊÊ?£ã¸ú:?Ü)ÎñüBl?¥Éü%‰?'Üqiú›?ŽÓ¿ªl_?ë«D¢'ˆ?·PŒØ$ ?½ð¾'m?´ídGj\F?œ´~ªÞn?­:½¯gN?ÝT2À$Pu?Í'+aœkö?àpBª–äU?ÌûÅ#Ç@­?¥Ä¬Ò4?˜È¡ô?ç»?¶p·E?´Ùô´ý‹!?Ë¡Üúþt¡?³\bòâŒÝ?³}I•'øu?–œw
¹?ٍÂá;™´?¯Ž|?àÉu]ìG?°´2§;MIXED4FGL J1331.3-3818¿ì˜ŠÛD@7ç†
¢À;›í0ðcÀ<zÝ¢w@€?ÐOŽ3?ýç½f?àEw¾}~±?Ò€U$õƒ?õYžfý@µ/â›Á?ïœÒhî#¿é­è j¿â–-žž¼¿Î±£Ñ€ç¿ïhey×\s¿ë_oÒ UNASNone3FGL J1330.0-3818?ïpM'KÁ?ƒú‰WYé?k%z[co?aS‰=û"?#\`ë?žÅÕ/]?ïb«Azê?Œk½‡BPž?q1	DoÄ%?tÇ큨=?Ž¼«
'ýŠ?…ÚúO €|?îÔd=TÓ?'Ùh×?|"p¥!"¨?zuªÈ\L÷?žN£s"~w?Ž"—`ªã?î.Š&´õ–?…P:"¡CN?x»®lC.?eÓïùqg?©ÿû|§_D?"Y¨˜$I?î¨Wc­é!?™Îçú½°V?}÷âZî°?s´`"ªŸ?¡»y«ó?—V}¹^óæ?î}ÁBá&?£¨¿-?€«®á±Œ?‹SCLo•?£ù,/Á‹<?žŸ‹Ø8~?í¼±g§À4?œ#B?äž/?…‡üa…™?göÑ.Ž?®Õ‡G'W?™pMJ)§–?ë~(MbDª?¢Î‡dã¯?}5´¤Ž?.y{É$y?Àï‹o¦0?¢oyÝØAGN4FGL J1334.1-4154¿íÊëu¦Â™@4@Ùè>B[À:`˜I7wÀ;ýːŒªž@¸0d÷¦j@é̂$2?À˜PƒÑl¿¬6ð/U?ç¡»Áâÿ@ɘ
²¿ïðG€^?îqu‹u•¿ë\dŸ¼ÉJ¿âj´>`ß¿ÙyÂ,_Ú¿æÒŸ½J#UNASNone3FGL J1334.3-4152?î©a»[á'?£ð «D‡‡?|ŸáåW
?w'u…ä?¡Õè‹m¦?¢êèùu™­?ïƒû:?yGQc¥	ó?S iw~ñ?^™»ß[ô?yvÖaÓ/?tmñÛçª?ízÏð‡?Ÿ'e×Öi?Œ‰ÏTÅã?‡1úÕÇèÏ?°žG—šñ?›Š$J{èó?ï­ï'ó³?y¢x¯Lý?o"ZdՌ?Wò,–?™¥þ¢tîñ?wm'´››Ü?í]Ã0°Æ?®¤…¯!®5?'ê-À3Š'?ŒÁÕë	/?°W[J~,?¬r¤9z?ïKyì]¿V?"p	Ú·3?iâæ!´?~ ò&h?"Te¹Áwò?®.'p?굗÷ƒÖ?«r²À€:? +ßôö S?"Ù"FÓªá?Á¨%'O'?¨?5¾'D?ík´¡ö?•l(¬ Ï?‡==3xc¥?w'ÖŽG.?±¿b³¬ÔÛ?"º¶6í®ÃAGN4FGL J1334.6-4435¿ï÷ê,"|@1šP?³t6À:OÜ»WZÀ;þ†
˚ž@HÂÁ@lÇß'Bd?ÊWvßZn?ѤÃ,ºô?úßú Âî'?ùJ¡¶×¿á§úð̆V¿ç­czù›b¿ßí´ctn'¿ípÜá¿ÝwGʙ즿Ð}U–4ŠKUNASNone?ê"Ãtg
´?ÀàNšþÚ¢?èӼ˺ã?‹ԕ"fK?ÃÒdñò C?À]¦¨š?íDZqžö?°^qIu=:?špn¤KÅ?Ÿ3%ù‹]?¦L¡/š_X?§Kì'*‰?êžWBd²?¨ÄˆÑ}ê?¦hø4V4D?˜"V!tÅ?¿ÚÁ,/³Í?¥(&®£=ž?êoí6µÚÔ?œ©×b#¡ö?™8Ãl±)?€ÃÍBY¿?Ã2¶¶Šì?™ëÖ6ß¹Y?ãf÷·Ë͍?ɬÚß4-"?¢Ï´ôîóÌ? ËáaѤ?ÖØñ\'í?É{ù,sž?é^h-eé¿?Ä3«,'Ù¨?¶îÎ\©U?¼&ç4ª›?¾±Æáü4?¸*Š›Þ?åØ@'†Í?±'M<´?·ú¨,x?£Boށ¢y?Ín¹z?­"­™Ê¥?Ầq:Í(?°yöJ¦k?­eò ¼?›{ç!ÏÂý?ØÞÏÃø?¯$–ˆ#AÒAGN4FGL J1334.8-3856¿Þ«ßÞ2¶ó@7("Æ£½àÀ:TqËõ6xÀ;í½îãx
@^¬ÛA@0!ùO×?ÁÀâ]Ø£¿¼jØE²?û­N'D?ú/}F'?ïôòñ#Ä*¿é-€¡{k¿äºïÀÛå¿æRuþ´ÑX¿ïöö¡²lÏ?î3Œ>½*UNASNone?ïSt|?žÓ~¨Oí?'õqÄ,?,
‰–£7?"úæÂj"à?˜!¶K:—Õ?íÂ}_k[?½³h«BÁú? :I:Ò&
?´Ÿ"Üû«ù?£àÎ|ôI?¯
^»'¶Ó?ëÓGãnyÛ?¥£û҆¼?¤Ôú#å:ì?œNÕm]»?¶ûCѽ¬±? õëܵâ ?íŸ)7Ô$&?"}p°ð?"8öP?€	…\
™?¬~¥ã¯t?O%öíYK?í¥éEuÍY?±v~ÆáO? \PœÕ­?£Ž\4vÞ?¥EcXTÂ?©'Þ¶í?êRvô—ÛÃ?ÅÒÙ ˜%ü?µ1^-†Æ?À6K»:Œ?¸:ê.–ó?¶*}Õ&d?è³f'Pí%?®–>XEàa?´"Œ£î°m?¥æ0ÌÖ¦Î?Âègé7?¥NdsêTê?èý·{Vã?²‰Pj3w?°Èç8Sœ?¢›¿~ND?ÇH$¯ÀU#?¯:]ÕæTAGN4FGL J1335.5-4546¿ïÛ·"Í?õ@0ií9SÞ¤À:Ao.ŒÀ;û~ÿº_ã@÷ `ȗ´@ßݵR?ÈEF³î…?ч¾û¨ØQ@5]¢r†/@ÔPXÝè?äčc*qÄ¿ÖÛh›õ¿_¿å"øD÷¿æ"6 M}a¿ë½ËrY¹°¿ðUNASNone?é2
úÿ?¶¦5¿Ú"ï?ª¸'ÚQª?š«ØI¶^?ćñÕ´–º?´'åj.pL?êeÎù¢Ãº?½ÔŌ-î?¶d[õO¡?²)þ›?¶m,;¥Ñ?³Û
3B˜C?éÂFzÒs?ªÔÖÌ°?°\r£‰Ó?œí¼?ÁîȬùë
?¥̼`âÒ?æ"×V¥?›ÝDCoÏ?»ô2¹³þ?[3Šúx	?ÉåzÉn?˜O;u£¥t?á:2cÝþ?Á*&àû"?À
Ž
?¯ί³³â?Õ~)üÂx?Á7£Ð3è?âýzPlî°?ÇöZê(¨?ÎX"gP?ľ'Pzþ?Åõ¾ž
ío?¼5cŽV?ãÃòæx?²‹ô°wžË?¾¿(@Þ8ý?¤ð
Í%À·?ÐÈP#·rÑ?¯ðG6†‹?ØM¦yÚj"?£§LöØÙ?Ëi\ØüŽ?£ñýî3Î?Ùý«§N—?§ÑI#ÙMIXED4FGL J1335.6-4052¿ä¡Ÿ:Ôxy@5;n.±Ä3À;^bMÒòÀ<…ú¯^&ý@!ì¿	ª@Óª6ŸÏ?Æz}ʆ –¿ÁÚèÄO%?õ-§¾Šà@ƒçÚ«?ïø˜,²²¿ìCË0ëZ¿ÚÌù"@F¿ï/<=Èã^?æÐ;·f3;¿¡Aµ)ßUNASNone3FGL J1335.2-4056?ï.Ò©"ô?¦ØEèÑ¥?Jö)P}R?b¸o¡dEz?™N?ƒ¯•?¦q[ɺ?íùÇÌݾ¸?»¦üiٞ©?þ™ô–i?¢¡Á`{ù?«ãܱ6èK?ºŠñyï?î
ÓÚuÿ?œQ¼ý?vo^?€Ìô;Xø?¬'Ô|¶¸M?šï
Ɏ?ï3òótxÅ?Š,YQ	oÜ?0¿°á?/\M«I/š?™>¥"Î?Š%§?"?î'ÿÁ8;}?¦ó>xî?Uû"‰µ ?TNTiÁ<.?§ 'Pœ'­?¦¸Af±ø§?ìàúˆ5²Ù?Áъ)l¾?‰&Q·O?Ðu2büð?µÓ[Ó?¡Ž?À12i¬
‡?ìóÊVi²æ?¡¿µM"a1?}»I†žF?'öû¶ ŽB?¶…øµ°fë?¡"¤7,g?답ηV?²¢¿W=g?V£à}ÚO…?^úôÒI>Z?Á£á™K?²£«)œ®AGN4FGL J1336.5-4655¿ï¼iûúÀY@.}â:óÀ:Akn
#ÕÀ;úž#lÓ@?£v'-•@éZD4"?ËZX¦ŠBå?Î[Ähû?ÿÓ8§z¢@ú…"áQ?Í&ý…Qc¿ä,È`›±¿éšãEµ¿äAÃ^¹ô®¿îq‹'æÎ×?È}+å6%+UNASNone?ì飭CÅ}?©¹3ì*Zþ?œ¼5ú¨?'êã}LJ?±­3Š!o?¥NI56?íÏM qÏü?«åº)h ?˜Ò¸Â²J?—¬iݒ?¦¢9u?¥Œ¤}è?ìF»oú†;?¤!c¦{?¤`ßµO5?–™õn?³™´£Ì}'?ëm'׏?쪟6¢º'?Žy8â/ñ›?˜¾¤ö"?s™£DðJ?´{]JÊ-Õ?Šq:-[?è¶y'¢õþ?ºXVB×Àò?²UT·"§±?ª×µ¡ ?Ãûqõ´ð?´Ú"_v>=?éèTC4nX?Àь"æk?²3ŠA[Û?²áS‰%?¾‰Ó¤"ƒç?·&RùAâÞ?ç«
eÀ?²díëUy?»sæ=6A?©`‰¥Ø,¬?ÅçÍäÏÍÞ?©ý¯
È?ærÊRI#
?¦|ž³ 0+?°ÙËϓÿæ?'{¥åB¿Œ?ÍÇð͐Ÿ©?¤>Uð[ñAGN4FGL J1338.0-4159¿Ü"R@4
šÃeDþÀ;
ÔoX}À<‡µ¡7Í@  ÍâK ?ú²?'ÌÎz?ÕòÄMã
?Ò¥kŸ`X@(‡€'a—@Ç°-YÕ¿ïöÊÍL'?횣"Ôæw?֓åDè½C¿ß5î#‰œ÷¿ÍK€†ù¿éÒ%œq».UNASNone?ïæËlÌå?[»7'Ø#1?9gg7}Û?-ÙçR"ñ?fÿ—<)¡?YXFî:?ïÛ¶&Ã
[?t¤šÑj|ß?BÁi	•E ?QMÆ4"Ë–?o™~ÂVêÜ?qåŠÝò&?ïU5¶'›?ˆ{@Êßæ?bu¤àFP?h­$Kï?"
"¬Àò?‡Dœ1çh5?ïœMł£?e§Ú½	è
?BÁÞÁŒ+P?/skú¹þ{?‡Àžæìzë?e
5ŽYUü?ïÈFdW1Y?püÁgï?IõÇÇ¿fê?@'%t|ùy?xžÝm"?mÛõ*Ú4B?ÕÕñ?ˆèEVÔ֏?Ui-"‰-?eŸúaP—
?‡$äèÇ?†!äIk¯?î %¿Vÿ?•ŽÑ¥µÂÖ?jLsöò»?ol¼ç53?¤XßãQ‰æ?"Òú©Íðî?ï·JtI?''M?G_ô֌·?A
·ma®?›®½®?Eur£V¡AGN4FGL J1338.8-4509¿éóÂ"µó©@0çm"BJ'À:·)Æ¢ç À<6,ém"@MCtôɖ@ËHûòTF?Âü¼Z
è?pý
~Êeˆ?²y=®ŒDò?øà‹ÓÞ9?̙ŽŒ"Ž?éêô€­¿ç

Ÿû³j¿å¨šÞ"Ô¿æ60ÞÅÕ¿µ8äx0JUNASNone?îÚÐsÓê×?¡õ¦m¬E?fU:;‡Œô?e$WSˏ? í¥äÀÂ?¡&žþ?Púó?¡¤zÛ(à=?'ÿË«¼?"9û…d0ì? ;*z1\?Ÿx¸Êø'k?î›ö~•j?"æe©_B?z/6DѾi?ywÔóðѲ?¢ú±Q:=?"‰²€L??ìËlœû?r™iaÝ/?–h–Auk<?w~èR¹?´
	Þå¤?Š³2ëfu?ís LëYï?«Rn<,?{ý0>B°?rŒJeNÅR?²§*à(?ªKpó†j«?ì½Sb}£š?´}Ü/†t?–>GÔxŒ?—ù÷Ä?´…Ó&Å?±‡—ˆç'"?íBÆÕ?¡~h‡E1¢?ˆQ¢ú¸»?'	@ÙT"­?´Õ
ü~Ã? R~ò?ç¢	±?¢é>¸ñza?ªýtVsœ?"C W"?Ê8db!ª—?¢'óÄ܉AGN4FGL J1343.5-6827?dÜEÀHŒ°/À:ËCæÝõÀ<,Mâ"s@=;"@óÅ¢6 M?×*Ÿ[$"Þ?îÍ~d^N@f"»ë@;(ðÁ?íÛûß	s¿ÖAcAî·Ù¿ä(³GÀˆò¿ï춬Ï×C¿Æ¹Ä1r¿¿ïá½õ™t±UNASNone?Þà֌
²-?Èh_ÐJ/Ï?¡6(î{ƒ?S쬵+ü?Þødq)õ?ÈŠh#U?áÞ璲?ÉËޑ	A?¬
	Z >?®'ùüÓ??ØÀ¯,uK?Æê)@¸yP?äIˆÈø1?²Ûö™!?Ã5‹'¢?©ÝE|Ae?ˤÇP7š?­'O¾nÝ?åvhDÀî?°S›6~v?¾J¤‡3f?ªû²k›?ËSšº^"?¦'V! D?ÔìvÙù ?Ŝô'{¬¸?§i€÷Ƨ?¤VywNæÏ?ä3H#Q¶?Åø*ü?ÐøþàV}¡?Ê{ìñ––ì?ÁKºS"'Ð?Á'vQ"v?ã0'û»?Ë=jaÑ3í?ÞXo4bª'?´ÜL?̩ֈbd¤?³¡a³%?ÓR¥‡l#?±ˆº&Á…¨?Ԅ;N	Î5?¶V0vô¦?͋§fit?¿—õk?ܵðþÁwÀ?¹ÏÜn!éMIXED4FGL J1345.9-2612¿êŠ-ZM ¿@A‰:'£SÀ:¹Y×êðÀ=£.mѕ@©t$j¡@Ç<t$•?ȋË:PˆÚ?ïþƒ~$H4@&\âY&@	>èŸf7B?íPŠ\õ¿ÚrÃ×ZÅH¿©–Ú]À5Ì¿él«úÅ-œ¿ïÿþøþ"?ïj8$óTUNASNone3FGL J1346.2-2608?ÐÆ+ýxªû?ÌÈÌþÜû?æýTÄtÜ?Í×Ì*/\?"ûµ–ÅìÃ?˜QÅI¿Ÿd?¼ƒžÛwàa?º»èŽtLƒ?ê7ӛ?ƒp?¿…No4ýI?±½ÄJù÷ž?¨Çà3UÞ?Ø°•ŒÍ6?¶+Ü@¡õw?à܌\ç"?¶4äBº?¶YFè"¼ä?£i"̳Õã?ÙÔTøÍ(?´ñ…bÜÂY?âw>-•Ã?µo)êLI?§és¨l'?—Ì÷
>â&?Ð?xÍŒ?Ê{ß¡ˆç?çõƒ
#?ËÅ;¼wG¾?›}X$tÛ? 0­®å¶G?¦üFU,ŠÖ?­–X8Ԝu?ìvt»é¥¡?ºB0wÓ1|?°Î6ôd¿"?±Ó¹ÅÆä¥?ÓªfÊ©ã?´Ƀ¤â8?ã"FȀ&?µ®"üZ'?´µÊœñ½È?¢˜èc"™?¸ÂÑSø®?¦w~}颷?êèç
CXx?°›4žyE?°™ÞI?£ÇìQóâPSR4FGL J1346.5+5330?рUw£@NÜz¿¹¾ÓÀ:h™î˜ÏÀ<ž))Äõh@œ³ì+6å@ö"ï¾i?½–Öñ"×?¹6w‹QØ:?÷W›ÈH@§¡§…§?êà^úâ4¿æËÔHµ{¿é€NÚX¦Š¿ç!ßeUÅ¿ïù¼º0¿Ù&ðކßUNASNone?ïݤ~'š'?b›ÙÒ|3·?Z´%2ªÒE?PÞÈÎi¼?enûml"?['ØÞ»#8?ï="MŠ«?š~ŒÀÌZ?…"Rü½Ÿ?Ž}å0¼x?"g&uwµË?J"¬W§Ö?ïWXÎß]?ª·½0΅?s²Av–Ú?r-e_žÁ?1q[Ó§?wÈîõ?ï&µz1Á?{\Elç?"*áAÙd?xûñ†Í/?{ù¼C-Õ?\2¬Ë¯Ç?溺ª–?xûá¥[u›?rÏ¥%[1¿?g'êæ"Y?yZ²¬ó?rmG'E?íƒÃmlXÞ?°‰A<á?˜ä£Î¾Îä?¢/NŠó%¶?«Qw>kn»?¤Ìr쩐?î"ó̸LZ?'¾¦"Ñם?"	2¿@?~ÛTe
-o?¡®v‡‡""?Œte‹'Äs?í²Š}i?Ÿeã,â@?²{0‰ˆõõ?'DËC?•üûß?|¯kt¹"AGN4FGL J1348.5-8700¿áh«©ÒÀ8;*'ñ¶'À:ˆ cLÖrÀ<2
˜à66@ô%8Kv@Ô¼÷"?ì˜ôX,¿½­‰:¦Äû?Þd¸[¦™Ý@	D&{Ÿ^?Ñ''?X¿ãáÚ{9¿í^lœáL·¿ïþÂþ—Ë
?ïñhÃ7ø•¿ïÿ'ö֌UNASNone?ëûv«Ô/?Ó}…ÅYïh?ZSցÚrÁ?Ž‡OoGï*?¿»¬;?Óhî	Í"!?ïÀ¨¹óh?½O}×÷?Së'Ñä7o?mÊì–Ïah?z°Ù¾?Œöˆ­Åñ?ì@•ï•ú~?§·äÛöÜ?'$±Fò?‡«'æ2S®?»¶º^,¨w?¦Óæˌ?ïû¢^Ô?7iËm²>ÄbѬDÊÔ>̀ºóD?AcK¤*r?7]
'çFÁ?ï5ü‹	?¶)HZA'?_UÆiÞü\?Æ (Ðù?—Xä,é%?µÔð6o?ïq»C.ö/?¤ÔO‡x?[òD¬Õ?x(R`sRö?	mňéQ?£h–¬ÎV?ë6N¤a?¬œ8e5n?"±¿êä?‰ó^«à\?ÁÞª®'?¬É¥BG¸?ïíñ›@ì7?gí°u'Ï>བྷ¾?ÜF`Ã?aý§‹v͆?fÿxæAGN4FGL J1349.1-5829¿ê'Ä5N–f@Rºû15À9'ðrÄB»À;TkJѵ@ÇÏÿZã@ù†üÞãP?ÇSÖö·W?½0Ãj¥?ö"fÿéYË?ûr—w*ƒâ?ïÿûÎBÓ¿àxŽ¡îÒ±¿éñ×HPѪ¿éނö ¿Þòb+‰ò¿ïš¢ãÅ6ÖUNASNone3FGL J1348.5-5833?åã;4o¯?Ã0!t³Ÿï?f܍·É'~?\&
E6å ?Ւ€n-Ü?Ã*:?…À¹?ä>ÞhZ ?Á˜Áú®(ê?¢~iÞ8Æ? :üWäIi?Õ2uóø	ç?À-œnúÎ?å`ªåœR?±9Ùø¾Éþ?°Žˆ……?‡2i5ƒ?Ó"5ÁÐ;ä?°´jk#?ä‡F.HÎâ?¦7ž#'kI?¥[ˆÕs?…B@†Ò2?ÔF"X6ù?¤ÿàåýX,?ÙVGÆy\É?ÅðÙ3.øÞ?r‡1í¥f?h,ºwýhÿ?ã/ͺªØ©?Åö¹"uÝ?ÕJÖՆ§?Äèì[;·?³%¢8}º?´õøníò­?âõàNVF«?Å@T殗¥?Û´ƒt?µeœ"´*­?©µl®µý¬?•Ÿ«îÎ?àŠg°úo"?µæÚîÐ7"?Õùu]$H?«8üDæb@?³É©	É?›"ev˜¬?âŠ@$!6J?¬™úý²iMIXED4FGL J1350.9-2757¿Í÷[¹¼û@@ŒÜY1ÊÀ:z(4Òo¤À<Ç]!CG@ÌÆHy@‰@¢\›âI6?Í{±ýºÃ?Ðé̂$2@;#Â|è?þ9—ÒÅ¿îðŠ!«¢?ïDŠ=Ü¡¿ç®ùþY¿á)-÷¿îk½Þrf¥¿ïìœ
!¼UNASNone3FGL J1351.1-2743?ìÁSb[G'?©?Pw±+?ŸIÿ»R3?"U•ç;³?²"å	
!?¥>}!ëlˆ?ìF-,D<×?´´ZÔј?±qóCvP?¯ó?)R?¨~IQÅ©õ?œŽZ_Š?ël'ù÷±?§M1ýw;U?¦ù
?	…Y?—HÂ(+?»°£?4É?¢Î©|M¢?çËhYìÂ?ž	Q¥sž\?Á"Bâ +?˜´ a'õ?Àޏ{ø7Î?"®úç­ÇÑ?è±ÖÐ~Q?¹åžLS7,?µÝ݉y?ªDþøô?ÂI¶?Ë$µ?µb)ã ?ç#ŽG›?Ƈ;Gºæ?ÆÍ@m¶ð?ÃVôX÷<?»ÙM²UJ?°w?V»?åñÑ<"Pî?±Íxl-€?·q¹ U?¡ßi¨'`s?ÌÞ>†šÜ?®"~^¢<?Þ»¡8@ۊ?ªñ£&þJ?У¿y?¬ Tè_b?РŸFE£g?¦‡ð]w^ÄAGN4FGL J1351.6-6142¿àԆ°fmP?ÕÃí_êKcÀ7þ§vÑîuÀ9òzƒSÜ÷@Î$ªYZ@(H¾µ²Õ?¶>$'ýu?Ñا¡o%þ@ƒ(ùôMD@n,"Þsé?ì›Æ/#Ùú¿¯¦^B¼¤¿äÛé B*G¿èõ~ò¤M¿í3nŒ¥•P¿ïÿúVrÓ\UNASNone?·ÑÕ`1R?Â_ Ê®m?âfmmýŤ?Î%T/N™?Õ>¯Ë¼5?ÊÁƒ'
?ž–´UëA?§WdVl?Ùc^"DȲ?Ã1A@'?â]|om?ÃâãÍÍÜJ?Ám­é˜ñ?±ñ¾/m?ßÿՖR›?·ëP¹‰§?Ø9)54ž?µ·i'2qX?'êÊ6¹`?gC#<"c|?Ë]"Û™Ä7? ÷éhoM?èÜï µ?¡)éY0¯?¦T_Ñy&?Ä⡕'w6?æ'~@]úB?Êwß4®]?Ð0w"Ïe·?Å5d¡?†#&ÍS˜I?ŽR
¾ÚpÏ?Ûä|NÉÖ?É^s¯5sf?áµm¦‡ÏÔ?ɂ3Tí?´º@QÅë?¨½Sô?á•ù|Z?¼Žµºâi—?ØÆCø
©r?ºTö–8ªÛ?`Z2L³"?K¾(E[Gï?Ñ.ô5_?­š%ÀåÖ?çX+Ë4ò%?­®·lv}MIXED4FGL J1353.5-6128¿çˆrn¡7?à´¬Ã˜À9­ê‰v6À:DmŒËU@ !€
+Œ¡@Ù\T"­?ÑÜ©ò­1?Ð¥·_'WÞ@–ѵ(k@_ƒmÞ)ì?ïQ½ei¿Ù¬bÉù³¶¿æÍØÀË◿稊-¿ìèÜy¿ès¥J_ UNASNone?J°c›Áù?JFzLr?"²¿c
n÷?–vÄÈëm?îp'†¨?¦sjG%ì>?¬˜æ)4ï°?´'n.%?¦"u…ó\?¦'ŸkŸô?ìÍ0ÖQÏ?¸7­‰n0é?ÇÖ¼&ƒÄ¾?­oKäsÌ?¼ÏȈMŸ?¤ddU*"?æpWåUjý?±w$ýúè?¤î!âý'?"šPLl?¢O«ãƒ?"3é<ø4?íŒ#1]p?âª þ¼Ú?™–nŸx‰\?–RrÚPu?'2ñPX?'‡¢žfb?î«
óNã?¢I5°¿dª?Ÿ#`ÝYo¯?¥9æìЄ?§Á®-J?­Ð4¿³g?íŠÓ¸EΎ?²ˆ+3ê¦?¼"%?ÊÏ?¡ðN3ÏQ?¿åÁ²´À?§4Ou°œ›?è"@¿?­y¢€¹qþ?†ÿ@VK*?pÕ'·"©?¡a1©]kr?\x—dŒÒ?èMS<?ŽÑÌ"ôDãOTHER4FGL J1354.2+0353?çvr¼ÏÃ@O,*^x[[À;]ôiÉÈ6À<®$´ë.¸@ ͇‹z&?ÿÄXŠÑ?È[XjËP¿†¥VøE‡°?ÀÎ2èà~°@9ÂÌÓ?ïðp
TÙ¿æo^݆Ž¿âWʌ€¬c¿ìI!ñ¿Ë?ÔÉÛÁ‡I¿Á•ãšzUNASNone?ï^›Ï&ª?¡ÎÉàµí?RÆ
UªÉ?q(Kd®©?"-4\!@?¡—<fötµ?ïZMÙ§¦£?™WJ&°<?n¤>¡Åô×?}~FüA›2?á¼÷V^?"Ãeè3§ð?î¨i¥­pˆ?"Â
¯ï?nm­Ÿab?t+A¬™6?£'NÉ÷c?"½Ì5Ø?ï x%U¤ø?pÝû¯óf?>ýñøHX6?5‹	˜s?†êqVA?pÈ¿OuXÿ?îÚ5¨zÕ?Ÿ	·«:q?`VDÐS?Zë!ù†]?¡YY뮺?žzMø&.ø?î³-»
hË?¬…R«A¹h?r›´)Ôkþ?‹ÁtÍÚñ?¢y­ÇÍ)V?©äÆY9Y?íÁ>föŒÂ?šù›sÁÈ?túŽ$f(ã?u˜'õ'¸?°¦cå—Cà?š2ëào^5?î^Ù |Þ?–dž²ü?\]*Ö×ãb?\~­žº?©/†‹Œõù?–Y1åúGAGN4FGL J1356.0-6747?Û«PÅUÀÄSK×nçÀ:RebZh+À;Â)©FµÇ@¦¿Ë1—'@¼¬ùÈ®Z?Óˬ¦¼—Ë?è-3¿Ë¤@yl$ìH"?û[9i®ƒ?ïFòbˆ‹T¿Ý½<‹÷p¿ëXd"¿íÁED­®ú¿ï¼~Æ.£¿é—€ŸÍAUNASNone?Ê9fF8§?Àáæ59ÙÒ?·Ò]lƒ4?³uÈèhi?æwZÀüñ?Å`P«FÉ?ÔѵÛw=?È=^°9™)?ÅÓr:Qõ?Á1Uôp?à""–}ãä?ÄmÀÍ»	?àøg
?³ˆÿ :?ÀZÿ 3¼›?¦ÏqÒ18þ?ך`¹0ì?²I=krð?ÑÌ#¾ ?¢#ÁäÜûþ?Ù®œ‹•?«Š¹~}?ÕO?¶×Ì?¤üRŠ13ä?Áéڜ·û?»U؊×E2?³jL¤Y°?®µhÙ½ˆþ?é?ÄæúK?Á¿Y|GÇ?ÀâØ&ó	?Á­8Ãý?ЫvzI‹ÿ?ÈÕW±€ý?ã¨L
Zíž?Èÿ)Z0;÷?ÔS°G"?±ôÂþûo¹?Çþlñ´§?±hkš]ñ?ß­º×ñ‡Ü?¶T-üÆ?¶7["l?"à`+ìv?ßz¬çï?µ<E7üøb?Ú÷}<86ö?³J¦4ʜMIXED4FGL J1356.6+0234?Û4+M-'@Nt*€JÀ;ÂÀð À<Úü›ÇqC@úk­ø÷"@ë=Ñ?ÐmÝvV?éºÅ˜ûäè@ô]…TÖ@ûlYA:¿åÝlÇ©w¿Û É8Õì¿Ç8ÖöœT	¿éŸxÁ1ãþ¿ïÿÿ" 5•?îƒÁ@&¶£UNASNone?ãOFtâÐ?Èl![šZŠ?Ò$éÿb¡5?ǐ"	e?¼ò$[e<¬?´dÔ@v¢%?ã˲ÅSu?́!0Yí?Òì<³SmÕ?ËÌÕ®ü4ø?µñw'çJ?©·âM]?àðPyâf‰?µ¢¤ïUF?ׅG2X?µ–émWÌd?ºh]÷×è_?¢ÜöÏJmœ?êőw¿²¼?¤)K­òNä?¾)1Dύ?¡ +iqOý?§T…ûB†+?ŽÔÁç*@ý?ÝRês¯X?ź\O꬏?Ø8!ÂÐþ?Dz0–m6²?Ä붥v¥+?ºZ‰õrïr?ÕŒœí_?Ëû¸ï0‹?ál{#•d?ξœ—i­]?À<ú7Ð7!?´'󊲾?Ö³	¦¶§`?·]1™·?á	jÓĞç?¹Æ™
úáÕ?¼è'´èL?¥'ßêÞF?áËKæ2yz?¶ÇŸÚÆø‡?Ós‰?•}?µÄOĜ#M?Áì£T¶ï?¨I£9ºèMIXED4FGL J1357.3-6123¿î»¯ÀÄÎ?ސpõ³ À8ïåÍNÓÀ:æ	´´¨@7‰Ia@ŠR¹á7¾?ËÛ)†âñ?ß[_!M­ˆ@þª°BR‹?ÿžwì©·¿á$rÀç¼<¿¨}ô]ƕâ¿ÖÝË!Ñáà¿ë·†Ÿ@øn¿îÿãIœV¿èD?JÑUNASNone?•Á` ë̱?›Ÿ3«`èä?†eãÝi?‰ÞJ¡Úrâ?îø`ÏM°? »×µr¸æ?§‰·cO'?®QtÇ9'?¼TÈü€?²ß–.ÿ<¤?ë9õ¼|•?·~¨Ìbë?´ƒ"©oÄl? ÎáòEN¶?ºÇQšžÉ§?¤ÉzER?ê£WTòî?ªÆŽØ:?'M]œaw?xÙ0j‰?²Ý&ó³H?"ó§îK@©?í趸8k?˜§l¾	™?€1zg¢k?J+CæäÅ?'æƒÌ
¬˜?kèbKò?ï(ø3û'?"!ÍgùÏ¿?—p,F»î?Ÿ#Ï4}'"?¿±0:«?¹âúÔ¥'Ó?ëTIü7Û?º†ly½?«2¤?•u,"ð?¼MДØ0?¦sºëVƒ?ê¾4}$ß?©â—D—Ä?q+ÞIÞ°¤?`g
',?¶Mrü+G?¢ Š-"Êq?íþ"×#N?¢ŸÆJÐÔ[OTHER4FGL J1357.9-4907?ït¯ÿ®î¸@(¡™V}»À:ÜþÒ—À<¨Ï—'h@¬Æã#@¿Åäë?ÅÓ\ÉY¥¹¿ >ªhR?݊´cõGë@z²ái<?ïÿ< A¿¿æ…¢×/ý¿ì·¬ª–¿µM`:—¿è*øÒU-¿Þû¶YÃÀµUNASNone?í¯?«'"¼?´ï¦À+{D?g í$uö? 8T϶?±ÉšŸgµ?³9^ú?îVҒ½?­*½‰›œ?qbäîÚþ9?wd!º%Z?¨fz5	Óè?«çR4*T?ís(5u¥? ·xQËNÈ?'IÂ×V™º?€ƒÜŽ£Ö»?²…ùà?ŸÈFº«`a?S¼ã?}³CÀEi9?k&u£°Ê¿?SàÖDzéš?œÿi%_??|
5x$,?ëÛÐW¾$`?¹ÀLÙ?s!"T]¹?…éÒ=»R?¿ï»,nük?¹8‡ï*Î=?ëгÁZu9?ÁK,`8Ø?€'zG	 ?'²jiãðì?¿h2ªˆe{?À¶)–Áñ?ëñ–þC?ª'CôF?'w'–¾`?‹ÈVwYH‰?ÁmIPù94?©Ðv˜Ð?ì×Ù¾«T‹?›Ýhœ
Ì£?ˆ¢&
I½¶?y»-YE¾?¶,íKåq?šy–ÜàG&AGN4FGL J1358.0-7749?Ì	°7À¶"À.Ök\šÀ:{@¶©tÙÀ<)ŸY@J›÷lÞ{@̳_=}9?Ìu´øo½Ó?Ç{V¢ùê'?üû=ÈK^?ø))ò—·—¿ÄÏ8
û¿âs~&÷f¿ç©>RK&¿åãHÿù¿çú¢'ݔ›¿ïÿ/‹_UNASNone?î†TGÕ׍?©ÖqB5Ð?l$x}½·…?lQBb?¥Øs÷ƒ
µ?¨
Í
³s•?ï	Ÿ
>>Ì?—íi$†È?áþ®³«?Z›EÚïi?•Û°Ph™?"Óbkü¡?î™yëTt?'²7¦\?†#CV4ø­?'ÚvO²Û¸? ßuÞ–? ×¹UoË?ës·ƒÿg?Ùº^Ã? šÚ¯‹â?y±F›È?¼ֈ¯³Ú?Œ#+Hñ?ìpËC­ W?°"ÞõØڃ?'KØ(/g?{wöJ6gk?º0*Þ-¥Þ?®"¤±&ˆh?ìáj+u'A?³‰Kéû? «ÞAs¦?¤å¢È̟ò?°­Øµ¡'§?­L¸R\è:?ìÌuÐwãM?£"®Û20Î?›8€€í?"+M¸O?²Î1YßÝZ?ž–Ö=0Y†?åX0—f?£¡_ä%µÅ?°üj¡Ãæs?"®aóR,$?Ñ»$¿ä?¢R<­˜D©AGN4FGL J1358.3-6026¿ïã6¯z½?õƖ^¤ÑÀ8"n°'-À:d>XˆW@x=û»ù@‰¤Y=?±XR&"g¦?ÑyYˆ1'@@@&`½?ÿF
ñ/W±?îöø_LÁ¥¿Óîtý­ë5¿ãKíÿ¢b¿èÉf@¿ëÓß ¹ôX¿é3€`°UNASNone3FGL J1358.5-6025?'{¡¿‹yN?"8OøqÞm?ä&PiØil?ÏÿÔB?֛¥ßåó?ÏÀ¥ë¯L?'XHX˜ÏC?žü>¶f\j?ÝLN`ƒ?ÇËO–Ž?àÏ1»†JÕ?ÇežÝZä?¼}¥PxF?ªÆ»Ú,?á\gMRTr?µ ë|Î"[?Ö'ÈG9?³…x¡»¶?šÍÖu?p'!0*Û?ԂÀ&ÿ¦Ç?¤)ܸÌ;?åBE-Uè?¤vÖ¹õ)™?zˆâ€R÷¥?|œ ýdí?é{zð?ÄòFPh'n?ʹËZ8Â?ÄÛÀÒåâë?€H'äß?‡35–ͧâ?Ü@¹Õ4‹‰?̒aŠCþ?កÍVÐ?Ì¡Ô0n\Õ?¨`™¯ÕJi?žW\Þ8?å죺¸UÐ?¶ÝEa
U?Ñ¥T°'ó?´à~yen/?k6"-øJz?S;9Ò?Ø.qh´?°A$J}¡?ãÖ¿Ti8Ô?° s=êeGMIXED4FGL J1359.5-6615¿Ñ;9«·HÀ&0"ÝzšÀ:wŒ 4RîÀ;¤»5˔@Hàø'ï]@yYE³Æ?ÆÅÒG5Ä¿¼·^""m?¸ßw^Ü.j@ú\­U
N?ïôÊ(,o¿æР@ý¡+¿æ'³áÄU°¿æWæ`ǖ¿ËTO£uœ¿ï¤œ—zÛhUNASNone?Û4aþÅà?ÆÞȑ˜ˆ?mª.Zý;?_ùÔï
oü?âH$Òló?Æ*|
<™ä?åÉì/
&?ÁšEÊÿ1?xÑ98ö?'ýÉl4¤?ÔãXÕY8?Á<ÒvãiÐ?è¦Í	ï ?­øq8£öÅ?'ìN!•	?"ðwjÓZ?ËC¬¸þ?­%Û§s0€?쮣.BÞw?'¬[]áÂ?h¾Þ¬,?Qí?¯%›"?¹Ê šPã?'}–Û%?Ôw±šõÃ?Ãý×;¤Ó?y†ÓEn=…?pì–%åý?åÊ6€«È,?Ä"@UY¤?Û!Í6ÌgD?Å]!gÐZ?xôÏ5·æÄ?ŠyE¿ ?â=/Æl5ˆ?Å-¡Æ0Gé?áÌ?YîD'?³šÄS£ãl?Ê|á3(z?7AŠn?ڊÙ}4^,?³†Nu²Hb?昗óɈA?©[M Ë%Ô?×µ•Äéý?q¿_šu‡?ÒOqBô'…?©2V+Ì0MIXED4FGL J1359.9+3616?îÖRpÿá;@R5!…Æ~À:¦ªWVþêÀ<"웟-W@+èJ%@§†
¢?ÃٚæuÀL?¬jÐa	Ñ?â%ëoOC@"N0"Þ¿â¹_'F–½¿ã¨"ÿÔò¿êÀÚPC¿ïØ]ÂRö¿î媞ú'¿Ü¿³O÷9UNASNone?ïä¢ä=y*?f<z`—?RsñJÏÁÓ?Qiq¢Ëm?b#"뤕¬?a ¤Mé¡?ïy5'\ªë?ÅdÉ¢?o	 öÔ¸?y\òt©+§?‰îX€9?‡±(¢"¹š?ï8ÆVLN?Œ'¸¼Ö}?wÍR¢œõ?u]<'s³?˜%'ˆC¶?‰nQKŸ?ï~õ!j5?sc%&©?"+®Ús~}?p!T¥%b?x.Æp?\†U[‡~O?ïÙ }?pWH
ýC?a'>æI'r?a]ŒŒc¥À?eW r@?hX…½m®	?îWÌÜ8?«Ôrã–J¬?†"û'ËT…?šø5iÌ?¤é¤OÔI[?¤U·ãև?îpÕØ0¥‡?'ʤóLºÚ?ƒ›Tg/îì?~šƒ-'S\?¤ÍgÍ$Ô?½{›ã¾?îh"÷&Æ?"……÷Œz3?ŸÜ]=¼±É?'Í ¥Ti?" ª=­j?~¥üBJ=AGN4FGL J1400.0-2415¿ÕQÌ—Â@Bt§qÉqÀ:B¿ö$´ëÀ<}+é'Ö1@%Ù}_QI?ûÎ:Ufcâ?ÃÝýâŽl?ß(Cëè@fX`f@ŒÀ0Ýž?\X¿Ô¡—Zû¿Æ.·ùVº¿ã[ãU¥N¿í€<›'Á^¿ïË!6±mUNASNone3FGL J1400.2-2413?ÀøÙ+fy?» á\"n?êc(Ñ°a\?ÀR>,FÁ?¥ê9JV?¡Wc)*?dž•ƒäÑ?¾"]:vQ?ç36Þ¹^[?ÀǸ[%À"?·YÖ	*"?«'Lú?Àþ'(±Ž?©¡»Ž!p‡?è'ý¡^'?°=ˆÝWá?¹k¥aa?¢mÀôb¤ ?ݯˆìa?§IP^šÉ?׋ÿc^/q?¨è`Ԑ—f?'nÚ)+È[?™âŸqØB?´j¤H%1?©ÛðH€a	?ëñ´Ø[Ä?²óˆä?¨œ#篵?¡-Ñÿ<?¶K犀[Œ?³ï£fw?ê)47Õ?½aÜ``	w?¸kNÓXÊJ?±ÊI #?®Úœ·8ïh?žÅÄӀ±p?ëZHvnú½?ªÂlÏº?µÀmð}¾ã?¢œ	aWÒ³?Ð@'˜'·?§½\ë"a?Þ>tz%`?³5_Íä݌?сíÔ=?ªû
¡aËMIXED4FGL J1400.4-6050¿ï2IÀcL?ìóŔÊ'À9·ÓôzùÀ;CÓÀí@l§"W`9@΍F¤ÿÿ?Ѷùü°À'?æ†\㔏@wàmò@ÜòJµ°Ñ¿å>, òÔH¿æ¨!â}ä¿Ñ}Ýï<¿å.	"&¸Ñ¿ïÿý`éNä¿à–
~C›UNASNone?Âà54j?å?¸ºE¹š+j?ÇD¿É?_Î?¿¸,}r­®?åvÂÀ•˜?Ä2=â0-½?¹Q"ˆ'Õ?·˜<ÆɗR?¹ü'£Ý
?±!ì#6?é´­ÞÂe?½L8Et[û?Ó^¢¤Ò6?±g[Û2?Åw'ÁCŠL?«U«B¹c?àòÍýEÝÒ?³÷)¡‰ß?Ï7}‹­.?¥L–˜ž¢?¸+ñž³÷Î?™^4°å$W?å,¢i;Å?©ã²"™¶_?®óH4íµŠ?§¹±',ï"?ƟΖ?`Ø?À@º|µ?èh××ϒ?Áæï*ù0Œ?©ZÉaHÊh?¬2¸!å›	?¸Ë/¿¿ï?·3¢Éâð?ëPíx
u?»FcÞï©?ÃóÑfY•?¨e…äݚ?Ãì.FºN›?­":}ÚjR?æ+7Õô?³»þL?µ7ÍC6­Þ?™$VёæD?»?%€~PÏ?¥«b|žw?éñ!¨Њ?ª'l±P'àOTHER4FGL J1401.2-6116¿ïZÀETóÍ?ÞQ%ʟÀ9[(5©/9À:Ób¢Œ‡b@·:ööìÜ@ª`üšò?ʗð!:¸8?Ù¿E» '@
	_à:gÛ?övàœià¿íD]Ä×5?¾æ]Â}ée¿Õ˃ÁÁ¿âÎòJ¶Ý¿ïDá±``?£Œ'ìG-UNASNone?¦"»Ç>? ïI}¼2:?¾ß2*·{?¶ôWÒM4ÿ?ê»!o
?ºKÙ:vüê?£I]6ÔâÍ?ªè+g«Ã?ÁkƒÂÓá?¶ÁÝ-Ä?ê‡OK†û?¹ð6š'?Ã}Õ:ÑÚ?©6¬ ˜¢Š?Åé'^®Où?«¯$å{‡?å¦X³·‹?±ªê8á?­'PVùn¾?‰å"K?ÄWÂ8
&s? 1!x/BŒ?éêlV%¸?¡Ü/9€3ª?¢<*Èh"?"oÔúޙ?Á¸TþŠ	?¹…==¹y'?ên;þš
"?ºí…w˜W?'µxû?˜ÃY×Bä°?Ñáôý˜?¿"Öw¨?ê…ÞµÇ;'?¿Y:êóº‰?¶3ŠºçC²?›ýϺm¾?Æ:0fǂ?®ûcøST?竤â‰?° "¡?<.<?rsԇ…À?ÇHÑ¢Hâ?©™
t}O?é·ÅŠtsÖ?©úåÒÁÔ,OTHER4FGL J1401.3-5012?ïëO¿äd¢@&Aòý¸ýãÀ:SQ÷GËÀ;åF­czú@1ʨZR@vÜB‹•Ë?ÉŸY¢Ò?ÃsÇ¢ìS¦?öO²$ªÚ4@›±vÚþ¿â¡{_ò®ß?ïõ–Ÿê³¿æ¿a>ß8à¿ä¾É¿Q9.¿ì¥Xtá¿ðUNASNone?í.:Êp?«†WøçS?'³)gÌOÌ?Šaå‰mbÀ?²!_SÖŽ?¨±™«èD°?î­mQ×?¦Z-¡b‹œ?'?
%¿Až?‰Å7Ø•%? ˜EÞ:ñ3?¢ÀðÁ5ÏL?ë$oKšæ©?§,s7›|è? Ø4q6ä?'Ýl%¼)?¾pkk¢Ã?¤"íœ×æ?í	¦è•2à?ŒEî0P©?Ÿ_T¾.{?}?(@Qþ?¯µç7Ä?…3Ý,_g@?éš³a¥?·`¥ûv?«­%v2ìy?¢<ñ
yZ?Â
KÕ¸Ñ?´'€9«…E?ìYðHÝ&?¹rr›x
?ž˜Œ	€_Ë?¥®ÑkñTf?µŠZ»90á?µŠpfA?æ늮€l³?±"Aˆáe‹?°AIö¾ð?ž/ þò?Ì1¡§Úû?­Î[µ`ß?é°|)ú­ä?¢€Ï÷Ž<O?°%<2?"_×Ó|n"?Á+å=?œ×wà19¦AGN4FGL J1401.6-4645?ÝÑt!N@,×`Ï‰@À:_!©ó›À<Á±æ—y@×\Q9®w@æ¤ì´?½x؃å'b¿±=Þ^p?ó{;	ÁIâ@·•‡U
¿¥ò¨ êé¿é
á,ˆ¿é//˜sÿ¬¿àC݊¿ë$®ÖAÀ•¿¦&™áÔpUNASNone?îÙÑÏãO?™Í¦,A?t•v©êq'?h"#c'ìd?Ÿ h[W@c?˜—&º¹UË?ïÁÿpö?ŒLH	|?c8þ§¤ïð?h­"'á?ŠÁ@'¸ƒ?‰–×Gz?îkúûfñ¯?–ãÁÿëèY?UÀ›Ïök?ÿÓè#…5?¤êà#ºÆð?"‹Ï|`•ð?ïMk
˜"?p œ9Qpc?hŠ½o¡ø]?MédQa?"Lºõˆ"'?méiôæö\?ìƒ\ým9Ð?±…»¦'Õ.?ÏG¢í/?…ö¡.#Ùî?·±F-$À?°lÙ£ô?î¨Î ¬??¢z0ò¶øA?wtiÁµ š?†»
,©¬6?¢uæX†v? .^æ~õ`?ëÕ篕ô?¨Šã&0?˜ ½½IÓÝ?'þ5 Vê?»("÷&?¤k'þ7-2?íµé¥ï"?'îaí¼Ï?…¶MšÂ­r?qJC§Â?¯3ÒL_÷Y?
‹ydR·AGN4FGL J1401.7-3217?ét§L4¶ì@<EB€®IÀ:½–V;À<x¸Œ£è@WrÜÁb?ýTyð'Î?Õó!à¥q¿?ÖÂhż7S?û\ߺZç@QG9Oó?ïyn‡P¿çl…>õ!¿âãÊ|"¿ØŠYàœ'¿è¬¦Q8ø¿ìžÑÿUNASNone?ïÔÜj›÷?…Œæ>.û?Qý7GšÁ]?`à@ÌhÃÍ?q|Ì߸&?±à›n9?ïÖ_áÎ!ó?p-è*:2?GŠ°BfUt?Pðô+ƒäî?qÞ¸øþ…·?j©³œìá?ïUé0…®Ö?ˆLÓ1.ºí?p,‰µЯ?r»ƒµgç?'7·È2?…jÔÍ0Ñ­?ß4GI?eQñãêŽ?bã¶üŽ?D÷êh•Ü'?‰•ÏSˆ}?d±¯†ë?ïÌ£¸'"S?t7µ?WBrª8@˜?U
:)_]}?s݇
‡ža?p䙐Àó?ï†psÝs?ˆ¦ñ*F?[õééú˜U?fŽ)ÒKÎ?Šå&H?…1ÑìîÁ™?îßh-Äg?'hàË#®?t'<6†Ö?vÁʚ€dã?žòk<ÅöG?rÍÍ´Æt?îÔî€?'QÜIú?n¾ðcòš?`ÐֈÁ'Ò? Å7M?kQž·riAGN4FGL J1403.5-6236¿ïØE«bw¿ìD¤¿èbÕÀ9NûH
[À;ži9}@ŠÊ"£n@í÷­K'?ņIÖ©?ï›ü€¿@Žï¬.@ËÔ²IhÕ¿ïÿÝ/ñ_S?ïÿp\‰¿Â©•e,¿ã¼ì™.:¿ïÄaùð†?½•æܘqÑUNASNone?ŽÊ@'"ÞÆ?'ž<ˆ€›?ç%7…äl7?Ë!¼ç9(?п>óõt{?ÊAR}Ø ?šöñÆ9?§<ïl[?åÅliÆÔL?ęê
Ot?ÒŸ!Ú×?þ­ß:§`?Ãõ»×9ÀÊ?«yH"<àè?âºî!ŒE?³ˆJÞ<å"?ЏEÒ6?°¯QŠìŽ?£J0
?ç$?‡ š`[7ô?ééPÕl?ª§aòýý¶?È3µäþÈ?¨cì •šÞ?…d\cÏ?…ª‰R?èÓ;ë'?Èù•7Š/ï?ΆÆm¸Y?È|šdÛ?ƒ|a¬™¯?{³BM7?çe~#òM?È	
Ì,¥?Й"ÌïÃ?Ǻ\C#¡?µÂšòW?£™cPÍÆô?åU£5ñ÷?³ÊøY'•?ÏÈ<f°·?²	÷:¡¡?y@·¹¬h?iú­æíß?ìÈ,¡k?«²É\?¾
³-$·?ªøH>œÃ§PSR4FGL J1403.7+1513?Ñê#¨YX"@QZ0#̎À;hÙQ?µÀ< cÞÌ©'@A_ˆhš@–•3®?ÌOÈ?—Á"¤+1Ì?̒ ¾ç[ï?üŠQՃ¿ïÿÿ" 5•?ïÿúVrÓ\¿ç' ¤:\¿ãUGá‰ó¿Í–õåÊʔ¿ïÿ%¿Ø·UNASNone?îU3ÚM¶?°Èâa¨tO?ckéZ¾'Ç?f³Î³à¢W?©vI)ÿ?° Ø|Á7<?ïÄulàöG?yà ½•òM?L徶2?Sƒ³ùi%?zD­õnØ?w©¹ÙŸRõ?íã‰B<=?ŸÄN> {?'wΠé?…§ÛŸÐÏ?­B|êûü?œ¼è|>ç?ï_dì‹%…?qË41c?o]"«"WÝ?[²Fnh?'¯ù*Äg?p;ªO?í¦'Êq°?´él{åe?uãGʱIþ?wémÏÕ?±p2Xß?³Ä'"­ë?ïS&[?–åÀM?`aqÌÌ{?lëëÓ"©Z?"tTbC?"ÎÂ]lž?í-S¨Ò$X?¡*þ΀Þ?ƒ~Çs?")ÞDa¦?´% €A? ox;¨?î1×]@ð-?ñÍ<}Aœ?ƒ~̺	O?wÜæ¼2Xì?¨ü 
]?—H-AGN4FGL J1404.8-5237?ïáçOž½Š@!M¤¬ó²À:lÚ"À;癴qŒ4@NMlDvÒ@ˆ¢ù"«ô?Á6F8¨²?Е§œ'›ž@	ŸNÒö@+Å ¿Ë,a‡ÚTu¿ç¼"pdìê¿Ôïʓ6©	¿æÖÜH¿êþz#²Œ°¿ðUNASNone3FGL J1404.3-5241?æË%áC°?¼zs©¶?ºþ¹ë§?®|n•?Ê]vrøðí?¶"f\öé?ä"á§ál'?ώ‰×?ÿ?±èþ<€?©Ž>YyO?Ò^<.b²?Âq"}cê?æp{n©?¯ŸÀ¾æI?½k™A™?£ç‰§ä)?Ǹ\y
ï?¨›	³Âkž?èt	g²Â?™ñí·lØ?¯ô¬ög?‰4†8v–?Æ2›níà?–=«ñ)?Úgý}¢JÌ?ÁX'mqu?Ìóaðú˜Q?¼ žú	N'?×Q‰ài?¿úWõ_h?Ù`+'ºÈØ?É®!2w?ÁY«'zC=?»œwB	m?Ýòÿ‰?Ȋ‹B؆ƒ?à–Š¬§ú?³&²f,g?É¥«DU´+?¯@ûµÒç?Ò÷ýH{Õõ?¯/¿R"6?à¢Çß8pp?¨TãQá"?¿´J÷n-? þTòº?ÖÍ]ÁQC"?§0pѝmÄMIXED4FGL J1405.1-6119¿é¡ÑdÈ<Ö?Ò&Ÿ;š
À7€®I#À9iÞÎW@	¿Bu›c@PŠ"Ràx?±M
NóA?Ñ(6À[zO@"µz»ˆ?öŒ¯˜ß_w?·Ë¼V‡÷¿×ˆï]J¿æ«"zuè¿éç.þL²¿ë'®/RÓâ¿åï@4£UNASNone3FGL J1405.4-6119?~–G'[¨?€GÙu4/?Ø	h?jµ<?Ëí·âô›7?ã¾QmÊ£?Ëô¡à\n?|}ˆ"	™?‰Âþª°ç@?ã÷ª<?ŵt®/?מµc_Üñ?ŽKWc·?º{¾½üŒ?­g‡Sdå?×1eF´M?´¶Õ˜ps?á"æH?¶Ȋ¢ú¤?DƒTc"fŽ?0o®¤?ÒÎP‡´6?«n	%¡-?擷!¿ÃO?«žÝ\YK?qàµCº†?oÔb²«'?Õ»&³.Q]?ÈÍà'?å6䘛m?È&2àŽ0ì?s©x#.-?‰Dgr†Ùn?å[bÜ?É*=Zgj?ÔúW[ÓÝ°?Éë»>HÕ?²\ò€ê?¦²íŠ~ëæ?ص…žºì?·x§}$Fp?ádl9Ս?·ölÐB5?ff«™ª?¼`ÿ£Â)?׫‰q¥?´ÞÖ	˜w?ä)•
qP®?´(Ÿ»¯ŠMIXED4FGL J1405.3-6008¿áoóÚû<?ö«#/¯ñÀ:4äR´ÙÀ;^¤€}há@!¹ÙNehº?ÿ7½¯lj?ϧWGd˜†?³TÐùøT?åóÕº²@ò^ªuÛ?ì‹m¡Ä
†¿ënÁê»m¿æìma,j¿å!Á›Á<¿ÜˆC{)ìã¿ß]©~i'UNASNone?àèôjlý§?Ãçßú­?UÄÐkË$¶?Lmˆžá®‡?ÞRZ‹_?ÃéW²n|µ?ÖKÞ!«BÜ?Ïk ÝR?'OžÂ±?™1‰6‹\‰?äI®rÌ*?Îѽí‹ß?åìˆI¡E?±‰ø¸t6o?Q5&ÓSz?"Œ'Eã?Ó=UF¿":?±8ݔÃZ?äyWÉG?¬RD·¾=€?q~…ñ¸ëÍ?[ì!*	ýO?ÖÇ9›W4?¬mfëŠ?Ògúvdq?Àu	Y[ï?`qŒ%¥E?VÞÞ²R ?æíZç,IŠ?À~#9žÖ?ÆþSð'·?Ãà"9iia?†s#Á€?–o¿??éæžw¤Ò2?Ä5D¥¡d¿?ÚDŒXáe?¶¹Ãqv"D?›–ú™=ó
?ÉÁ—žôv?â'2Û?¶zŒ+½‹ ?ÓÜ6A…†g?²¦¾6BB?{[('[?tr¢¯ûÚ?åÛ-àãÛ?²ìÿ@i1MIXED4FGL J1405.9-1853?íêrÂË@DHFà!qÀ;!¦Mà^À<\m¿ <@ Ťö!d?ü;cž5	Í?Ô-ÁÚ*ƒ?Å(ŒDâ?ì%Õ²NœE@êŒÒ‹Óˆ¿â*"Q€ü¿í#¸Œíº¿À'\HÖ2§¿çKýî,￟‹råOпïÿþÞ÷UNASNone?ï'íØéª?"‡0ð¿™?P*'&¤'L?U'®˜v/d?‰?hÒz¬\?'ºÀqFU?ïÀ'ˆ¶??'4¿·¤?M@K֊i:?V¸Fê}ÿ?|D2=ûJ?€Ý"ÖöK=?îýµ½ÖT?Qêì8&?b\+Â)z?dyÓ¥¶âÅ?ž£ÉüÁe?|q½•?ï€7W|‹
?pÇvGï%½?> àvKÝ?-ÂÕþ-°ƒ?#?!ó?p±¦œ‡˜º?îÙa‹
_ª?¡+ R 'X?_õHìØÜ?_aÉ©˜É?¡l÷¡£˜? æ¡6Ö\Â?ïW&UæL·?"íŸk›?[WÃoݱÂ?i0ù–ˆ-é?"e¹ÌC?'¡žôíë:?íé†"];ß?›…ºe¦?mcaz¡U?ocü'®â
?¯'g¾L£¿?šå2ˆä Ä?îx0ªåá?ÇQ¥É"—?KIý8¹—?Fî'#œ?¨ÍYbèp?ÁÿåßàAGN4FGL J1406.2-7500?ïïÚÏç+À)²<êlÀ:§‰i ­ŠÀ<ÖüÑwV@Ðҕäƒ@¾6œt?m?ÈG<)¦íj?¢'­€™l?×VŽ®˜.?ûµ¯¬ÖbM?êŠÍÿ&ç ¿ééH-–;¿àHe)O"£¿ë›—jë0e¿â!iÂ;yS¿ïÿôa¼2¡UNASNone?ï¿,¾O¢?v£j—Ý/?D3ÏñÎâ?<ï=êX?}ã&î½Ë›?uº"²Jz®?ícp#˜O[?¶w¯ƒ°?s€e×X?zåíAÐǑ?³¬}ªñGæ?µºK7XSK?îor{ókr?"Xt«æ‡»?…A‰Ú7Å?ƒÙdžYÙ¥?£¸uƹ^ò?'k?<v•î?îy'q*ò?ýs·…y?yî×c©ž?`ÿ:(£?¥LË"è1?€b[ìÇ2i?îç*ÁŸ?œ¡^ª W?^õ5ì‰ø/?W¼°_2²? •ª8ݝÿ?œË*±?êžÃ7m?ÅnúÁt †?ë3´Ê6ï?ŒÊËùÓ?Äf@l½Ôž?Äõåæµgg?ì‹Û8?¤HH¯]?"á©áað?Ž!b­£è?¶®ÍGƒè¦?¢¨RÝ)?ëÈÁT@'?boÎÔjÏ?$Wúȧ?~‹ªOÈ?½Õj]Êi#?›^'ò
'äAGN4FGL J1407.4-0820?ïùI‡L@IÄ"`À:¹Š '§À;¶@­o9t@¦óˆs@W£TY?ÌYAºµs¿£ö傮Ï?̎EèíiÐ?ý 'ç´¿ÔîYyîÙg¿æÄe©¿á€C‡>MC¿î*Ò§a)? ^vÔሿãHû"±UNASNone?ï4´•Ñìz? Ù+ñÆ?YR¸ÊY?d¹Áü;Ê?—ÔLe6Ð? DŽ828œ?ï-@ikmP?=][k?x–žõù=?õ ߎ½h?"2néÌõ­?˜oÿæVk?êŽåAkc?«9ò¡øú?˜± ;7MD?'V3Š¾W?±lbî{?©?Ù»›íŸ?î4î³Ãn?':à[ýC?XFÔ|=à?OaÜfUo?«îÞ2o*?ö¨mßÞ?îº ¿µ"~?£Šè½v@?mã^.='?nI蕣ëU?¢Œe̵H?¢Ü.IÿF?îÞÔ-¶"?³õöòe7½?'›ìbÇÓò?'Jâ0Ê?ª •J?²#+V¯‰ý?è=oœÅóë?®i˜M}Ý?§êŠß2?›=LŠÉÒY?ÉÁsl?«SSÙÙÁ ?éï¶q@´ü?°˜°U/Î?s'¤¨ü?q`7þr¯?ǧéÎe¡?°]øSbùAGN4FGL J1407.7-3017?»°5R•@=ÂNY)gÀ:Á°\S½íÀ<"(LOcë@¾t@ꗃ>äA?Îþhö¹…?ë©hyfk@W[_¢'@ûr'¦
?ÅRHw=#L¿Ó?š_<P"¿ãT5â:\¿ïhD¿ïÿÝƒ(i?îœtÀFV¦UNASNone?ãái6`?ÆӐWÈá'?Ê]‰?{¸U?Âiëž?ÆÒq…?½œ×§b\?à"Ä*?ËVvEùÖ¾?Øìàª
':?ʍ…lĂ?·°a-[G?ª%×?šß?ápŒÕÄv?´ôaB©?Ӂ¥­Ûp?²®'ßܸÂ?Ã<«—røÆ?«¥¹$³Å?åÜFp}?¯Uvx.V?Ð÷½D?¬'ÎÃEZ??³Œ®Ø"Éâ?—¬CµñÆ?Þ+óh?ÆÚ6ËKËä?Ò}:¢W5?Åõý'èOŠ?έ¤'L÷ˆ?ÃTïnjõJ?Ët¦ë‰?È¥±Õÿ?åŽàøÉ?˙dÜ^ÌO?½…±I'€?µ O8ã?ڍҏô/?´1°7
å?ØcpŒ y?µ )J
î?Êyß%P-?±¯Ì›U"·?Ñ	"Ï™A?²¹j	±Î?â%3uo»?¹I(Ú=|?ÅX(‹'h?­ˆûe¿ßMIXED4FGL J1408.0+3834¿Þ´B"\@Q"-¶°`À;·¦ a4À=d2‹n@ ²->>T?ü̳¢Y[¼?ӚµUů?¾àŨ]_?î¤âè7Œ?ÿûR[Âsƒ¿ïږ";cƒ?ïõ·!iÝ¿çè§ô¦/ª¿Þ¯¦/OÏ?—øpƒd'À¿ïÿÒ³–šâUNASNone?ïÀdOœÁ?sÿÈzÀ)?N'ÜšŒÚo?JÔWh?{ý|«–Ù
?rœW'ÝB?ïÉÎsÒü?x®6}£@?Iu.Ýޚ.?Sv,ÆZ…?wê VJ0?u)œ­>?îø&
·? ÎLkÍà?f»h.uø?iK&ºîï³?ž#м0ød?z«œðHú?ï˜GµÝX?lXÜs1«?\²n!§·Ã?N"Ó=€Ñ?†c`E¼­?kuª7\Ê?ïz!5ÒZ?‡Ó%ÇÞÓ?bÏI¹d§?bº¿)HX?ŒÃà
Ha?…ÐfgZ?ïg°v]‡ù?'><hËw`?[ÈґÐD?i7-ÁÁÅ?'Md‰Ò?ƒ+†%$?îd?'	?™ß
FXŒ±?q•ÈÏË-ˆ?rª¹ف?¬Œà¡—Æ?™
¥V.?îƗÎD?Š<×
ýËq?n}OMW»?i#ÃÇ?¡®²Í ›ç?‰–Jþ­¤ÑAGN4FGL J1408.1-6010¿ÏÿeF<?ô¾C·å´ûÀ9¹™	PášÀ:écyL8@ o+ˆÄà@õþÚf"?Ðli_À?¾"PTVC"?ò^FtŽ@–‰nÔ¿ïùJ¿@ó?îÄgÙ--`?Þ"ZÞGô`¿Þ8_~¿ïû ŠN¢û?ï˜l]vRÃUNASNone?ÅS³ø%Ò3?¾Î'ː¦?'½`è	?ƒø:¥Éx?ê`~q?¿Nµš¬D?×f^ÛÏì^?ÑiÏÝ"…f?ž| Ði–?¤:¡­ãsD?ãXïÉÈ?Ñ>A©™?Ô¯Í8¾ž?±WÁ<]Å?µÇ¾5·?¢™Ècg §?âï)kç¸>?²†Ô}º?ÝW‹¨ÑV0?·h¤Tגּ?"™zåÏR8?~'MŠêÛ?à·nT­'†?·"YjÖ	?ºä@ö"?²ýG›5€3?/g}ð?»0ú*Y?ì&ºBËE}?´UvžÕ´ ?җë]ujÕ?ʯkN5K?¤ãÄâ§èW?³j˜‰"¸?åeÎ6Hð?Ë AÁòy?ʚät€§Ó?«}X˜¸í?¶Û¬LÝOè?¢<䌶?æ}ÑY¤a?°-Hš2?Ðu¨¶h?·é¹·|"?–êz59îo?''Õg Ú?ç
Ø©R8?¸þy8UOöOTHER4FGL J1408.6-2917¿ÞWÑÃV¬_@> í_‹ÎÀ9¯»åüjÀ< ¬Ö(–@$ë,ß1@æ'öÀ?¶õIB¿X?¶[âÿ¿z?÷`ýV"U@]Î_ª¿ÐUýfȌ¿ævA:\ó ¿éÅ(~#qt¿ëp(¡ß¹9¿ã²€áü}¿ïí'ûî£UNASNone3FGL J1408.0-2924?C¿-¹?Ÿþ»Ñ4¸?Wh[~Ãå?M×:·}"Œ?"/'3.?Ÿ÷À&²W'?ïN¥vê?Ÿþ…èôÙ?ƒÝ¦é€8'?'CÜ÷Ýß©?'ð"½DC§?''¾ÖUg?îÂæ¼Y"?šQ"bÌ<ª?–Uí©Xá?'6HDÛ?£8Ú¾²?É?'b'ü‰]?îå?9b?€!jË0X£?tŒñtßÁ?uùç¨<iÿ?'ã'âA)ö?qοís'ï?ï^Š0Ð`?•¬ƒ™6¤*?oÒ8H¨?jdÇ}t\?Mü.à?"óÏ
¸Â^?ícE'0n³?´`8ƒañM?›ê˜ÄðP?§»›Àóø ?«ÖZ{\ÓÒ?¨¿_íIœ?ì^Ò¼t²?£ŠVy—?¤÷±'+?˜õrØT?²©ˆÄŸ?›ÚÜ0Í:K?ì™ñ¼#? T~=Ûê?«Å²4ò°I?™pÐŒB?ª›2
'â›?tF;CêAGN4FGL J1408.7-3747?߃}{´^õ@6™Å£ãŸwÀ:˜³"&jÎÀ<`% Jù#@M"òiG@Os²Lï?Êz:°€?ÙqR=9œY@Wކ2´ˆ@$ð"ê¿ïÿû-2h2?ïÿÚÁ,/´¿Ý¢¿³Öh¿åø!ˆ¬6¿ð?ïý¡ñ&UNASNone3FGL J1409.2-3743?åT̅ª#€?Æ`×w0õ'?ȦJ¡l?Ä­Ùö¹?¯œD?¿<5®k@s?êÕ\èÆ0?ÂGÇd. ?»	¼þ^ÑX?¾U¡­Ô1?¬–ÅÒ"EQ?¥ºí#Êل?㰆;J?²Z0J+Á?Ȑwœn¶?­W$óã
Â?È­ou"èÁ?«"#{Îg?ìϜþ²Î?–4‰KMR?¨z±5ê?ŒPÒc6F"?ªŒ/.?ŠZ¸¢H§?áxCL?Èafy~¢?Ñ­öxAÛ?ÉWR1ë?Æîá){$?±.Uþº0?äÆM'ÖÓ?Ë£{?οìGD?ÈÈì°r?½ÌïZÁB?²%•ö•Ö¾?Ý­•†±œ?µ‰£"ä\µ?Ðþž+#Å,?³'8éÍÛã?ÑSÌDU‰8?²ù'}›Œ8?è¼Ró?«ßgÅfE?¸[ƒ#©ã?¢%N½) ?ÀàõÈ2x?£`ípOV&AGN4FGL J1408.9-5845c?ÐàÛ
9œ@õöº «À9#¹À;íöé@Ê«V™m@Ìhĸ*?Í.rýMž?¬ÛMîöBg?ä£þwiÄ@$ˆJ'Ê?êy]ïŸ_¬¿ä)™A,5¿êI °N½¿éô›Gð¿á)zLÍ8¿Ø'Ü]¹oUNASNone ?â=%?Þ?Æ`Š*!!õ?|ëÃa+ý?sC·pŠMÂ?ÛrŠáñ?ÆS;4ùÖ?æ2g šŒ*?Ãlb»ø-?"àºgöÿ?•c$p*h?Ò]%­Û?ÂR|Ø p–?áÖP»ü'Z?´\"χ¦?¤ÞùQ
"e?•ôFa®Þµ?Ù·]®1?³³š[<e?ç–3
9?£¡'½?†ûDS3\?eÉÍÿÐz?ÐÁ³O^s?£BŽŽÜMà?Ùôò},óË?ÅŸl©³?€Wn岕?tã½
TE;?âÄ)"rµ?Ø<.Pí¦?ÜW#qû›?ÉX@±dÖ?9Ç9‹…?¨ÔM<ÒKð?àê 
bOg?È÷4V–1'?ÔB˜[V?²ÿó‹Ø"Ê?¨ü­#ßå ?•§òItmY?äNéMòk?´@ø%'¢	?ÝÎ0>?¯"ؤò=J?•8_…>×?€GüAOBÃ?àË3Ãâÿz?¯ÂGåQ;MIXED4FGL J1409.1-6121e¿Ýmî{ÚR-?Àû>û…À6›¾7ÔÀ9!zÈóú8@ «:ðn@(Ôº××Ã?›à¢í€L?¯¼Žç™@Ù¿Š¯?ø¨³‹™Q¿ïÐýH•›?ïðò`Û+¿Ý®êäâ¿âÊâ|azn¿âݹNjÇ¿ãA!"µUNASNone3FGL J1405.4-6119?wœ?¨ïÈY?¡Ñª
â ?d/ò a£?"Lâ¿yéU?7Ž¸¦5?¢£™#‡V'?ˆý¨a*à?–W0ýô™?Ùä¯l-"?Êà}ùÕï`?âª	<dŠ?ÊíAª‹?­,þ
m™? êi ðŠs?°Ê `X?¡¶Ne{ X?ìì.›?¨þ˜ïøo?q¼"†ºbË?`"]é»S&?º›ï_HåÍ?¥f¯y>ö?ì‰êà31?¦u^‡çï?zÂ]õ_V?yþ÷6kÑ?iúfæ¤q\?o·‹œ?ﰀÝ_¾?'ßKD?€jŽ"Ôý)?Œ ùˆm?ÚãŒ7ÂuA?Ðq/#hS?âL©fýK?Ðp¸ò$u?«˜øYÏqp?Ÿ…rù?å?­Dù‹öŸ? ÕÒà>?ìr áÌä?§Ø2¬[°X?_LòÉ!?RCíWÁ8î?¿y¢¿P§?¯Þû-¦ì?ì%·t ç?°úŸ¥OTHER4FGL J1410.7+7405¿ìOj¸ýÚX@Dõ*™0¾À:[rðR
À<ojM{³Ö@ ú'WÛß?økŽXó·?Â_Tä³ÉF?Ñ
ƒÁkÔ@€Ò=Oè@ë3zQ¿ïÿïXz?ïþâ^.‰€¿ÒŽä;(u¿ºÅñ;lÌ¿â²€óZ€¿å"ãÓrÙUNASNone3FGL J1410.9+7406?îî¨é‡‡b?ŸzmlZ•O?–‰÷8{à?–¤[0Ö¡2?ˆ0±¥^[Æ?‹Ð¢ºí‹»?ï]N>žÃœ?'SÞ*k" ?yúsÀÀf?'];ބÏ?‹¯6ؼì›?…Œ°y›QŸ?ìRÞn5?§˜Ì´áå?²¹­ÍÐzN?£ƒßIJ]F?¥^ÄAÊ
?–Ϋ#x¸Ë?ídªN?û¸õ4?™Ÿq̀^¦?zý
…'?¬æv1®¥z?†ã\Îe'Ò?íÛíùºý?¦žoÏî*Æ?¥øRç¢sÚ? Š7˜Eý'?˜'›H˜?"##64E?î­Êþ¹?¬©¬-½Iï?'cçZq4?™¨™/ʪ?¦ƒ/—>ÂÖ?£Ðiäp
¡?éC¡$¨Uõ?±s<'ðq±?Â;Æde?­Î'»:?±kjºN"? tŸ-:?ê›è蚧?¡û¾_ž6'?§–Ós]"e?'õ2û£ü?¿UO	Iø?Ÿôւã\¢AGN4FGL J1410.7-5945?Ǜ_nœã?ùx"«ËËEÀ9þAˆ`ŒÀ;(šrÝm.@ ¶é—îâ@ît¢iKô?Ç éD&Ëq?˜ÂsªO?ÔãÂwß5@¸áÜò¿ïé|Ñö®?ïól^MW¿çô´±M¿ÞêJa".Ô¿ì	íT+Ñ?¿»P¥	qˆUNASNone?Ø«¨×Çt?ÂVт?'£RÃ?tÑ{!
?ãlDÁÈ?Âo迶R§?ލ'¹O?ÐCÊþt]?te0ñ?ž:,ßw˜?à5Ó
P?Ïñ;Ì´Îÿ?àvÉ8ÔÃø?³pîێˆN?§ª»ëS¸?—Á8øw©
?Üb£¹?³'¡Í£??æ*Ã;î2?¥µ³É¤+÷?ê.»5?sOÕx‹ª?ÒòY&{?¥i±ä-?ÆöØóæ[?ºsýƒ¯?êS+²F ?‹e×9&+'?é vW %?»XÌÇ—?×B?ãùAÓ?Éò;"¡Tp?˜#&ļ'U?©E¡úÛ
Ð?ãÆ×ë8ô?ɵÌ¢8,?Ð{ÚåÜ?°
4g^à•?°Üü6;?"šöЌ?å°Ws"\?±v&Æ|÷Y?ۛÀüÆñ?±J¯Ûj?œç:mVs?‰'*†9<?áJå®	?°ÞGJ¹¯MIXED4FGL J1412.1-6631¿ï—ŽÜžž^À™V}»ÂÀ9ˆ̼À<Fí$[@'—îž®¬@UÒ°Y?¼€ìब.?Ùlæ³'à@*
4›èÿ@âd×-©?ä9pÏuôy¿ÓkŠ\å´$¿Ø'Äãõ2r¿â¥,¿ü"˿Wz:Y¿ïÿƒ}ùUUNASNone3FGL J1412.3-6635?¡@Am'@? Ý<.ô#?íMw"?²ŽŒ1à?©í͠͹‰?¦Ÿ©ù?¾–íÁ#æ?¹¨Q©| ô?ٜ€‹£G?ÃEècùq?Þ½Ä3ÿ"~?ˆÂmï?»ný­P—?¦§b´Dª?è['hPp?°œc¦oJ?ÀÚæá õ?¦HRy%"?Ú«+S§?¤‡6úïÉ?Óߚ`O1R?£ÌU¥Q5?Ñu^t]'¬? b|Ò݉¾?L'±íð«?ˆ½¼0æ^?í×Líeëå?¦Žî]ÕÃø?«8z'?¢Z§>¾nË?ªÛtý¥T/?¬wè¢sæ?ÛL2$·¼½?ɉû¡¡zä?à¬/ÉÌ_?É;ñàO?¡ÒØK"k¤?"Ƶ†ŠP?ë¡¢è€e?¨xðîÊ`|?º	|•ý­À?£ùkÈ?Åå¡Íù%N?žž6nWö?Üx!È/aË?¯ )H×<ñ?ؕ
QæìM?©Ç›L‰MIXED4FGL J1412.2-6018?ɔù"]?ð-}|,¡IÀ9δ#ˆ›EÀ:ég•:H@!1د8D@""úÎg×?ÆÕÿ{&¿ˆ¤ÒK«"Ü?Äñê¾zN¦?þ‰×Í0õÁ¿ïÿYø"'?ïþZxòZ%¿çÊ9¿¿H*¿åCÈü]´¿îä£î‡1¸?ç$¯!k4¬UNASNone?µˆzU;?²ñ™nM?{í@Ž$@? B'µÁ1R?íåöO¹7?´Åa@ß.©?Êûf×ê&?ɖ29–­4?›ÂB|ž®y?¤ò0CÛ?è¡o©È2?É͍¶{@'?ÓøÀá\%ñ?±÷Íõâ\æ?³='ZþLx?¡"FÓ¶çV?ã›ú¤mÕh?±ú³£¦¥Ö?Úns ð Ë?°lÍÿ>ô?–ò-䧥o?€òp$÷x?â5+¸¯?¯ö¿¾Ü?¯ÌŒø*Üh?¬Èp&¯?ˆÄMzÆÀz?©W'Î9Ú?í %ú»r‡?²ôZM†ú
?Ä\ᕺD"?¯H.ºJ?žÁ
´`†?¬UË •ÅÑ?éò¿z©¿W?ÄF^;Ó?Dž8Ù»G¿?ªôzŒ?´¹v›Í,?£jh®´?猚šËrÛ?°÷悵º?LJ~Ûc?¬	XK !?žÉ­¥Ãˆ%?"ZVÕÓj?é'ÎÑñ–?­Ä/Êfù±OTHER4FGL J1415.2-5550?ífefÙuI@'÷na«À:—J4¹À;hoB­úz@^øÓeî@°;Ñgf?×nA§V?âÓïÖ½@¸®$kT@ÊÂOpU¨?ïë°½¢¿â#NžÉ"C¿ç9Á¢w8Ç¿ìŽÜajS0¿ç‰u"×'ù¿×WÝašy¾UNASNone?êó6ÙZú¢?ÁdÔbdÆv?"šôC¦v`?–ο"ÿr€?Á¿ÆzYk?¿¹ˆ³~ƒO?â'ÔÜ»"?ÃÅùèÇ]?¯º:AýøÕ?«4t9®d'?×€«¶þ?ÁP
+0Y?æÊÎÙ¨Ž?°êÒ2ùc?°Â®tsϘ?¡¬%	M?Ìsm_ÿÄò?­Wu¶$:?ä<E
v%¡?¥àÆ4õY?¶~}¨Z#M?"µØ_?:.?Ñçց4%ª?£ŸdŠžH
?äóÞ3ô?Ãξ¬-?³îŒ…Ìí‹?±jøåÆL?Ñ wâÃ7?Â"©«¾?Ðï~M7ì+?Âß©øÃ?ždµóR¯?¾kB‡þ«[?â৬p¥ž?Äb"îÜ0?ÜÍÚºê?´N€¤£?Á\ôBî£?¬–NÊ3,?ڄ÷#ž§?´Ÿ OØdÃ?Ò]{Êëe?©ûym:G?Äå˒KWÓ?­árÔ¼bû?áÃÞ]‡´Y?± Yä8SxMIXED4FGL J1415.3-6110c?Ñå-ÃÔøã?°«ÝSÀ8¡=¼ùðòÀ9àÇÛÌD@ ÄÁ>ND\@ŽŒ:5…ô?÷™»È˜Š¦?ÄNž·Ëß?üG7|n¨@m |ŒÃr¿ë6qY´¿ï;	á€8?æëÂZƒ¿å®²šò_.¿î'lU"°L¿¨k¶B­àµUNASNone1?¦÷íYš)?ª¹AภŸ?³{ÈhÞ?¹PÉ})Ní?ì0µV…ë?¿´ˆ³Bb%?¶Ë¬ÄÍ,¢?¿9Gþv?¤ø1üQu?«`øE4É?ë×	dÝ%?À‰ƒÛþT?À,õ4'­?¨ˆwËM!Å?ÆAêeäáA?®gWq
ÛÌ?æhº(°Me?±¸9ë#É
?¯ÎƼ±Y{?ŸðN–—ÚÈ?rêÁµX›.?zìÝ£³­?íÝ>©<ò? ˜qô‹™?¡C×+†§¶?£Ñ)\RØ?².¼À
˜?¸m\{‹O?ì¥êõ¸'?½@@.e»h?³¢í^Ö?ºÛM¡©?«Þ¥Wáêö?¶åTN©â?ëÍÍÆ?ÀBÁÞ(·&?»>5£X'Ç?£¢€<ä'€?Ç$*³Ê?°±Á'‹u?æÔpA}ñ?²X×=±>æ?¢0ýª¹r??¤tzŠ¼…M?tÕBÅS?—Fڄñ@õ?î³EŸœh?§Ÿþ×n¹OTHER4FGL J1415.4-6458¿éŸø®R
À]±~'­À:"=n€À<Píè¦G'@®:»gʕ?ýlÇß'Bd?̛ŏÝ?áB!"9Å@Uþ9Vc@hZ‡`%?éHtxwàâ¿å©ÚúŒùx¿¶l=?üoR¿Ô /Jpfš¿êyþ(kB¿çy0m†XUNASNone?äÆTl*(?ÁURæ"?ÂûùyíÇ?¸Ñ;•"Œ?ÊγÕi˜?·1$4±›@?Û/ó1TO§?Äo݄;I¾?¥ös…ÐèO?¢)"Žlêº?áŸ.ë7?Ãû½µ™þ?ç[E\ÅA­?°ÀV†oQd?Áß'@>g!?©¯HJ£?À³ÃNÒS¨?¤¬$珝?çøϛD{?›¶Â¤sÊú?µO¿\¬?'íq?ÚÌÅ?Èþô᭞M?˜÷œœ<é?Û7¸,?Àþm¦$†?ËÞ¬ŠÚ[x?½ËtnM Ö?Öø¢ƒx?½ÐÔÕk.?ÆìÃý?¾$/	?«5µ9J]ù?­eƖBp??èÅ#$"¬A?ÀtŸá?á 6ô1Á?´c¬Ô)I?͘\bq?²ÿQªU?ËæË#‡ø?¬FÃHi¦7?Ü+8£	¯×?©[^rš{?ó%ÔnÃ?¨%3¥¥¿¸?Ùû4rèÇ?ªrQ:·	bMIXED4FGL J1415.9-1504¿§(dM1Œ@EŠo½'=\À:ä§0ž-À<€ÇÛÌD@e¸Ž|Z?ûWÓ[\G)?ÙoDü‰Rú?×8
2ˆéH?øÜz9'Í@"ô7ŸÔq?ïå' Pˆ¿íAýa¿§Ë.€à©è¿ãÂÜôb=¿æä–bWŽ¿ïÿ´JõǘUNASNone?îþûPBã?—vì±É°?eþO?Eº?[éþ'a?`Ì	¯…?–ï§4'R?ïbÖÔ/-?‡Ð£U‹öä?o"$Ç­ý?nw½çWð?iåèJÙL?ƒŽqfªó?îÕö8£W?–nk~ºV?ü)Š?­ÛvÜöÔ?¢£›˜O×)?'¿œR€3?íÛê&yçM?‡áë*Ç.?#1çè_?f3ϼž‡ç?­Þȹí¢?†Hþ.k8¸?í¯{Ä$:P?­AÝ^Ú?uGK¥Aì?p¤ì´J×3?±/­&³*â?¬Œî«ìI?îUfˆdõ?¡íÌ2ßU"?ɤ'å{?…xj€ï'?¦då
 S?žÏ-'ÀO?í$¥O@–.?£dw«¢í?ˆ[MÄí?'Ì"ls?³Ç*%Icí?¢!k,T?ëf5ëÿ?¡\`–)?ƒŸ2Wó1?xœ<ÏN?Á-:fý²? @æDgAGN4FGL J1416.7-5023¿ç|õÎ5@$mG8£µÀ9혮¸ÐÀ;øÂ!xÌ@ð·S=êœ@)†@÷A?À$œ—zÛh?Ӆ2ˆJ½@Ø.D¶é6?ø[‡`ﯿÒ8Àr×
¿Ú¬ìݎf
¿Ýê1!5.á¿æ
ÌÁå>¿î`ÊE3¿ïÿÿ&¦³UNASNone2FGL J1417.7-5028?Å«kÑèÉ
?»g-¶œ‰¹?љÊéà?ÁÃ&÷`Ÿ?áÈ@ØÍ?Åò"%'à3?Ô+<pëòÏ?Çh>i‰-?Þ»šÎ€‰±?Æ?Ý8ˆeG?Ê2Q'?ÀÈfoºfÝ?ÖlñAÑ1?±íá̀u?Ö9í2Y)Î?±ì	It?ÓY!‹ãE?¯¬ÕP?Þ8¼ÖE؎?£µ+–<à?͎©óÑ?ð?¡'g#9?Òÿî/чz?¢`ƒ°E¤ò?·høØgŒa?²¢ÇÔΟ?ÕÿW¨LT?Ã^ž*än?âa9Uâ
?ÅÊípþ'?Ä X8J?Áoӏ+#?ã%Ë·V¡€?ÊFA çÊ2?ÏHxê¢u¶?Å÷¿ÕŸ?Ì;÷0áR?®ÈÝϵ|¨?ÛƯφÿ?¶²®ŠäÂ?ÖT£àX?³Š>ö1‹m?ÍÔ"_.q?¢ßnß—6?Ôí€BýÍî?¯ýÄü¹?Ü(nŽ~˜?¯qHR
VMIXED4FGL J1417.7-6057?âñòSDÀ?ÆÊ#åbÿÀ9
>¼(À:G¨=¡K?@$x‰1l‰–?ý
¾4ƒ•K?Á…NÉf»Ì¿©ÂGBÒ/?÷€.>ì?ýîé':,¿‹?à<Û?îf^ê–¿î虱íM¿à³-ߌB¿äÊÜgtƒ`¿Ü'-ê
ËUNASNone?T®‡H{rQ?buXJ݇z?BKî6;_ý?N[·C3§?ïñÀËP?gèÝóœ?¥È¶.#«?²­ö¥Ô´?¤ø-\[Tø?­ädzPÎ?íSñÇXÆ?¸Yõs¯Ü?¿³sŽ±ÍÝ?¨¼ãnÑyB?¦6ÆÀ¸$F?šèH0ùК?ê¦%!çJ@?«êü§t½[?œ½æ0õ6?…¼Ã'Ðý}?›YÌ«èò4?£ì/åI?î?BiBJ?–IfGÔø?qÊæéd¥J?{Xg:ÅÐ?WXHÚÒŽ?eÛ	ïù'Ë?ïо
í(?p¤ƒ]?¦'ËŸ%?§yFF@?¦èsћÚ
?´‰é¹œ¸@?í¤H~kbF?·†Ó&—¿0?¹‰¾â+î?¤Žêšûñ?¢{‰#à?–@­'N?말+(D?¨ü'`?€¸"¿N4?s o_S¦? x""ù? ¿ŸF¿ž?<p~?¡kË
¢¿OTHER4FGL J1418.2-5400?ÏòLŸQ%@áÐÈ0À9ýH"Ô·À;}±CÝ¥@Š0NÒK@i"/?ÒzJHùn?܋AèÜy@èí¢/jQ?ø;O1¡¨?ÕÔ3~1´-¿ß{{áͺ޿è•.enâ¿ëOñå‹	´¿ïûÎ!á|1¿ðUNASNone?Üácò±å?Ê 'l"4?­áj'nŸ?¨dqXW¼?ß}ÿàè?Ë"zß²?ЋÞW¨w?ÃoG¸¸/?ÑGûIëd?ÂX¡úº×?Þ,íÖª°?ÀK0N–)ç?ßo†ò3Ië?²Ã:uôX??½}7kÚ¢+?¤Yѕyó?Ù1+3èîI?²pÔª@úª?Ê5 î%?š©-}•Ì?×^IْÙ?¥~Öå‰?ۇ?à?¤œê'ø™?ÐØ®Â˗?ÄÀaÚe'?·3(§÷?²§Û+ÙNp?ä­C›ô?LJ7®åR¢?µUs¤pC?³¿Û"—÷%?×ûyÙ	ò?Èæ	‰ÁŠN?áWÃÎvp?ÆUT¥ô›É?ӆ6ã
x[?°¬7ßÉ?ű¾ "?®Ë¾üFæX?àÐux{M?³ŠiPÖ¦"?­v׍E"t?ŠY,ô(&?ÛMã)ÒÙ¤?´C™¡(
£?à ò†ù7?³[ÃèP£MIXED4FGL J1418.7-6110?ãÿ[[àl¿±†SÁžˆÀ8!å±  œÀ9Fì\tu@ör~!Ãõ@¢¦¾EJ?àì){D?ÒXÉûa4Î@
% 8ð?øìWÿÆIP¿ïŒœ[ú?çÃEš>H¿è&@©-¿êcv'-"Ž¿í!­>¼ÿ$¿Ì‡´÷UNASNone?—ԩLj{?£…(´¯>?…iÙ(?"g	ÅӞ?îë³M'ƒ°?¨ÌDÔY"?£ q%çX/?®*Í­ú"?Àyñ_a?½·{Wº?ê§|¦ø/…?¿$oS¨?¹»sÀr?¤ ².ê7è?ÇZE¬îœ<?¯Y¼Ý1&?ç×&0Û?²l[Pü\?uj>Ä¥N?]6iA	Ò?£{7°zĈ?'B3Kôڏ?îxhhìu?'º¨C;Ð!?ŠÂz–ý˜?£'yQ¡Ü?ˆ÷§ñê÷,? -7D©Â?ï1uΟq?«`*ØaO?"ëþN_÷?žËPÃ3hZ?È]~O*$?ÅAa&ê?éS¯À¼7?Ĭ ;×?²b·º~Üù?à©&¹?ɀjòDß?²Àw>zäù?çSŽKÌuÿ?´bkÊ/aã?W0+'Oæ?H§°-ÑE?ŸèñEF?›ÖêæpëX?îüX¢rJ?›ËÀ]RÁnOTHER4FGL J1419.2-6029?ê´¼µ¨n?áöAÛl¢ÁÀ9"›vékiÀ:è‰ÁµB@!"|¨òýä@埱áŽü?سÑÞÚkq?'6¶ e©?ËÈWÈþµ?ü®¨Q˜N¿ïÒÒ4ëš?ïŸÄ UàÝ¿èçˆ9õÅ¿ä"ABÀnð¿å?¼xÁ²½¿íÜ¢ÞìâUNASNone?vÞ®¡"Ž?ˆa+OJQC?kDþø²? ©XŽ?ïfà€&(?¡!D&Ù/G?´áQ:XŒ ?»_Îû-æÌ?™ä~êþ˜?¢•Çi?òz?씱ãðÞX?¼âô–ë>}?ÃZŒPäQ¬?«ÆkiŒ?³3ƒžDI?£1¬ñ:??èÂìx'Ã?°:•b÷GÕ?¶"çâÅ
?—GL·Q?ˆi¤¡oê?v¸hoœ?ìÙüpÜê…?™öÀ©?×žüy?'ÅÑí_A?lsLkÿ°? Ëxl€åK?ïb­úy®B?£<»eNìÖ?±áàõ?³ŸB¡¡a? p—Òü?¯‹Ïÿͤ:?켺d%ª›?º1ÉH*]™?»ÆwU'¥?£Ûêƒa?±_¡7ÌÒ?¡þDù`&ý?ê[<á?«ù®j&³u?¡H"R
Ü?Œƒ¶Á8=5?ƒ9ËPgu×?}ˆoX€?Êß??"Ú'ŸOTHER4FGL J1420.7-6701¿ìLÜ)a"ZÀ¡©É'†À:ùp™ÆÀ;™oJ:¶µ@=1¦ì@^]×M?ÍmíCdٞ?Μ
!Áñ§@a&Ö.?ùyÕú
¿ì@r`ð…º¿Â¶YÃÀ´'¿çtè?ƒ¿ç ÄÍ¿ëY^@'7|¿ïâ[>ê÷ZUNASNone?Þ½¿5+þ-?"¬øql?"#̑RH-?±IŠJK?à¶3X?(+Ãà?ßúñ!Y°º?…(~#qt? p§Ÿü0?›€åÝXÏê?ÝöùêoӀ?Âé{ÀQ?ãS6͋R?²"š¿­7?§Q ¬?'¶›¬/?×g¨°¸Å?±ÑðÝÑ?âAÕK‡¤?¤'t3v?³çh
c?$\òŒ?ք;ïP?£Œøú¼Äù?É!Ô¤e-4?¹&p¹è? ãËåóÅ?®¶lc*œ·?赜™ÿ'?¼M*ï܋ ?ËqØÀ  ?À¨·Tü—Ò?©WÒ´"&?«ªs‹±Ý/?çŽ'¾òÖ?Áð²ÉÛ°?Ôn]ö͟?²›è€ï?²YþÊD"?šÉÐb?ã}²w®Y½?³B÷Bäx‡?Ò?Xpž?§HðA˜'
?¿«Ê¢ê¿ì? Î—ovD%?âêÚt*IU?ªÂs0èïÝMIXED4FGL J1420.9-6127c?烈^™úy¿Û T¾ôÀ9pAK#êÁÀ:oê–â/5@"Ž™¶Iþ@ð®Ý*?ÍÄn&NH?ªü8ö?è=Pù׳@{…UE¿ïÜ*7áï|¤ËüÃ5?ïø4SÅz¿æn'ûnj¿çnû€"dü¿Úÿr;†¾ÌUNASNone0?¦7n×XT?§—ž÷	]ã?r¥
fmk?gs‰"?îw?ì]È?©a˜vX÷¾?¿Fd/@?Ãé¾×ü?'§O·8Á?™.ýÚ»ì¸?ë‰ó•¨70?Ã÷‰äżã?Ë`Ü*ã®?¬Ø
"S"?¹¯!ɱí×?¨"âyÌ?åòÏ¿	Z?±Íʒ»?Â
¥öIH?¦d¬ç?vÁì-?I?oU¤g"?ëPy~Šä9?¦×Ô¤ÈÑß?¡ñхl†©?¡"hŠ­îe?x囲øÉ?§	Ý,­?íÜ?¬³²QÖ?¹š2¹Kø?½æýSíä?HK™¦Ÿ? ™ñ7£ ?ìWœË
–'?¾º|µ —?Â~ËÍseÓ?¦~¤"Ñ6G?·š#óá]?¨ÉNÐË?èm¬vëð?°ýÐOä?«‹`?°[?š÷åv´3Æ?vd]yoè?xéx5"?îÃ[R?œ½©Ð¥OTHER4FGL J1420.9-2431?ã¥"LðÁ@A¡ýiõÀ:^ÏO^%À<dëÄØí@çÒøŠì@ƞ<–‰D?ŁÂ7rˆ?È'øR¸@_Ô{í·?ùˆ¤~Ïê¿Ô²ŸÅ,Å[¿ág—ô}뾿ݓœº¶¿æ¸]¿xÑM¿äV›†Ù£¿ïô›]i¼UNASNone3FGL J1421.0-2431?îçÍòv?±Ü%¼Dm?tŽBÎ?…Bcœ•I?êµÎ«	´?®@ó%?ꑔú?ž¥^F,?'þ'¼[A?'G¥š©›?¬ÿúb'?'¾|SÂݦ?îÀÙ°F?'?'ÓC"E;Í?† Yx؉
?"·_~õç>?œ"A«\?ŠŽ{@X®Å?ì­³œÐæ?wԇ]*H?£~ímlš&?¨&ig?°ÒìdY¾?…],w:?í¦Œéê?¡óeOÖ{#?†Ü¢&Ú"?|üi"w+?¯àkOD¼? †ÎœÍÙý?ë§2±®
o?¶LØ\OÁ?ªù*¼«½??­r]Ð̨é?µIՁçë?ª'}u{8?íK|XQa?¡M!š%þ?™G¬ÃÁ+?'K
?®ª1Üå×\?˜òµ&®c­?èßxîJÃ?¢ËM é0e?³sª7y?—Tc$U?ÄFHGÜ&v?ž7ǯ'œAGN4FGL J1421.4-1655?Û&ï]ps†@Dj}¿H€À;'œ%eWÀ<¶´•žbV@"á]¶"|#?×2¼ë®9?âΈ>''ü?î0öã Ì(@vA……@f&ż:¿·Ø\wûT¿ï ˆ¡#і?ìIØá®a¿ïúÕ>
|±?ïöÞï@5¿ç.ÄÑ¢UNASNone?ï~!¬î?¨GÝ­1?lÔĤ0?¦ß0ƒÒ?‰JƛÜõ!?'Žn"É€[?îú퇋Ú?¨o|le˜†?{Òü·*4?†EûÚ"î?™ÛZHÑC?¥åQèzß7?í2|ùÂ?¤êì7??-?•püä¹õÒ?'㍡.?±Â,àEÀù?¢1ò†éÀX?ëÍu4¦?°²a9÷`?5Ží[ˆÅ?:®w=ñ—É?À¿d'îs?°â[MZ?ïÿPi?œ>ê?rö"U‹â?wå´úo°?™Ð[ûèéð?š¯$ù½#j?í®.vµéÜ?·ˆÌ4;Ì?‹¸.@kf<?žM¯Ÿæï?®/
†ˆ¬?´QӋ.§?ëY¹2¢OÝ?¯Ëÿ6EP0?—ê}ëEçI?'BÛkà?¿7–ðH?®$*Ê·|a?æè"R¥ƒ?ÂmCËíåÝ?1uÒ*áÖ?Dýá9Eù?Ò+v(®Óp?ÂlÔ+]HRAGN4FGL J1422.3-6059?í0Vi:£Œ¿¤Âþ*Æ[À8 6®è¶7À9­O©‹%@ FI²ül"@¢Ä?ò¥K´3xÓ?Ír‰Ië0@ƒðØï?þXËÁ	8?ï| ï
ê¿çú(»
,ª¿ã¼²F+]¿èëë†Ì7¿ìñ"b"4¿×r9Ù?¡ÖUNASNone? Ãr"ž½X?®>@!k%6?®$ÄWùµ:?¾­±²ÐÏ?í|'mr—?Ä#:Õòmú?­ÝFÀÏU£?³)ǚJÿ?«‰­u™j?®å!n™ù?ìiÂ°i??¸— àÈ?ºÃ¶£•›Þ?¥ÏʍjQÒ?È]œ±Y²W?°Dꕵ‰d?æ!ÿ6ßï?²`Ï¡‡?82ú½Æ¬?ys*À+'n?‰ñûh=B?‰k±ÔÎÎÛ?ïl'gð?œ>/?¥Õ}–?²…º•Ú˨?¬±m­¤àÂ?»NYX¥¢U?íGÀv°¿?œÅaã8¹?¢ ©3c±`?¨¿š»%Ý?±£TR—™?³àюÛ?쩊â`v§?¶F\¡§Á6?³5Õµ4Çá?ŸÔìoÄ!ò?Ë3wŠ¿ÐÕ?²š>ºÒ"?æÌgfõï?³m3oè?tV±"é?pfDmóAŽ?ƒ‰}ö…˜?– I'ïQ?ïŠéоžâ?–Iã4(ŒÍOTHER4FGL J1424.8-6536¿Ê‹4"§ßzÀâ[úҙ•À:&.gòXÀ;€å¯º@´ºÃ{@ÀLÁy²t?Ù>Nî÷ð?é2užÎ_@p׈§@&{Ÿ^?º,×#'×?ïè¹\­€¿ëÔ.béÚ¿çÏÚ¾|ýؿؓ²Ï˄οåÛíÎmUNASNone?Þªo)?Ê;Ëj³?£%¼RNU?¡S"ó3á?Þñ0MŒ?ʽ½Ó{?Üé-ƒÝ‰?É]¯çƒ?¯ˆ	ÖñÓg?¯Pw†po?ß%ÑE'k*?Ælf×5–?ᒵp©z&?²`>‹l_n?¹ˆíÌbö?¤°×Û?ÖxY«Ë}ö?±šR¹Ü?à™J6ãt?´&ÂѹU?ΪLUI?´5fêõˬ?ÎðŠÎòä0?¬°«¢éK?Ó!8¹Ý$?ď¤¼ýÏ?¾Fv­—ŽŽ?¸(Ýé©?⦔;œ?È_7ŒÎ?ÅÒý K±Ò?ÂØ缁?Á6Ã1SÆ7?¶¾½oæ?æ=Ë˜!þ?Çl»'ñ<v?Ö¹dÓÇÆ[?±¢?Áä6©gög?©>§€º?à*?ëÂ9?³4c×7V?ÅÙϔ¨C+?²C	!äA¹?Üï
†r¸?Ė.B?Ø$
°Kür?À½w¶+0ìMIXED4FGL J1424.8-8012?ärÎa!ƒÀ2Q֌i/À;¤š~›çÀ=IÄòø6@Fé—îâ?ÿé={‹'™?ÕªÜ3?ïÿ踻Ð@m$
<ÿ?ý^g×®6¿ç{½ ´ëÛ¿êá|¢¿·†ƒ'F>(¿Ù‰ÿöÅÅ¿ïþ¢½"°S¿íQ&ΠâcUNASNone?ãý²™?Ì>
ð§{?ÕCÌî?Ëרük©z?¦G½Ø? Û2Ç ½?àƒ›U†?ͽ§h¿¶?ÙDM«×?̝¯'0G#?ºbGÄu÷d?³¯¸˜?àʕiÖË?µ®N£bVs?Õ'«ÚR¶?´Oօqê4?†R¤""?§R…à‰€?áH_Ýƒ(?µÍÚÄÖ5?؃ï
0ÒÓ?µ,ˆ¸å~
?³­G[RCì? {O!hiþ?ÞýÀÑ}ñ?ʈںK?ï?ÛBÉe†Žò?ÊÓñ_º`ö?¶ý×$_Gô?±KF'p?ÐÝWkn/€?ÌÁ…s"D?ãRüQŸ°?Ð1Úö†/?Àý
7Ý"A?»LüTq=Ò?ڊö칄Ï?¸wߏNx?ÙÆXîpØ?¸?Î뀯!?Ç]`IR±?­ÂØó-?Ìà+cÛò…?¶B'9J?äD¾–(Jø?½×«^NP+?ÂÚA] ?²JûŒ¡æ$MIXED4FGL J1427.8-6051?ïBò\ÿÂæNh˜Å´À7™ʬaÀ9æ?Pwç˜@,ÚÏÄÎÒ@ùü£T-?´õæ °Ï–?ÅÅxDµ;·@9	ۂr?øÅqœ+?À)nä9P?×´ÿüz¿çÚcŽDÑÁ¿êÊ*ü-©¿åŠØ5¶›2¿à¨<_+߂UNASNone2FGL J1427.6-6048c?¸í]À>bÖ?µÚú{µ?¡;¬ôÈw? ã¶¸Ø1?ëΙ†í^?¸›øËĔ8?§a!‹žŒÑ?©¨^dH?ՙÕ<®Q?ÃaXG{?ã½I>@
?ÂN]!)•?µhÇ҂'n?£¹!C$K?¿"âl)°?ªD§œ3]?énŠÃy"<?¯€	т?–"þ±µy?u‹¢^?Ïñæ¾ È´?¦lÛBØØú?çNæZÅüØ?¦¢fR—{?¬Õn¾Æò?¦÷LÍð?¥Ûa¡@é?¢7JÔkzî?ìÔòùºÊ?°J°Ä>Äó?hÝFê
¥?—6ö8§?×t§¾ÅÎ?ÈÉ¿¾¾¹†?ãÂe6ªOä?ÈGeu¶Ì—?²ã;øIj? g%ùÅÆw?ÀƗ¶aó²?­iHÊÈ[f?ézªö8V?°»ùèO9m?w¥(´ Mé?a+ùD§Š?Ô=}ÖçÐ+?²¿sç¼
ù?å±öÃHó?²¿'ÀrÓ0OTHER4FGL J1429.8-0739?…bþȊ'V@Gìd^NiðÀ;fBÀ<ýÔ£Zã@X6hqÙa@UinX£/?Ô'Ӄ 3?ì|p(‡Ç@[bâMg'@Á*WA…[?íħÈ0†?ïó'?	*K¿Û&ÕøÎ]¿ä՛=ÈK¿íö9ãPœÑ¿ïÁPb#UNASNone?㟼O?Á@™k²'?Ï*Íýs?½fûj?Ċ³LÉo?´uÞfÛ´Ð?Ù*ô3ÝÁÖ?Êï;â"D?à9‰a?ÊrE¦Âô?¹‡æË/ü?ª²) l¯?åV‰{-6´?³j~¢«Ê?ÉÙD?
÷?°G-kªa?ÀÌÇÏ;?¤6eDä?ڛðÍnC'?±¯I¢?á$–rü)?²›lm~˜?¨×^ÇùŽ?'§¯¸¾À?Ûëä'ï¹ê?Á'‰$ßæä?Ö~'D´Ý9?Áì7-59À?Ë+èP¶Ñ¹?¹'Wï2ÛÓ?Ì͂¡§Òd?ÈÀž
—ˆ?äͅêe9?Ëþ.ye¹?¿øËi†''?³š¾þ³Ó?Þ²+šm?ºDa%VH.?Õ¢¦Ø
\i?»–,Ámã?ÇV[1æT?«"Ükwގ?Ås{ØhŒ[?¯öVµ¤?èD ×´?´÷
mT2?²ø_E…°?¡Gž1Ø
MIXED4FGL J1431.0-4432?êüjÊhˆ@-Ê¯¼ÎÀ:Zy¯ïFtÀ<"¢"=_@ˆ´™û@À#Uož?Òø®6Ý?ÄïäêOêy?òåQÉ oâ@ÉÎÖ俾šP£±uƒ¿éÔÎX¾7¿ä+¢zé«*¿×")ÛE¶n¿ëQ(¡´Æ¿ïñwÁØ}UNASNone3FGL J1430.8-4434?î¡ÑfíþS?¥tùW?ir®	À?_,̆"?¤K¾³C3½?¥9æhšÂ:?ï̔è§@C?y;ߪwÚ?JÀU¼‰y¯?U<=ÖùÄ?v]€ãï?u Š'-û?ïJføÔà?¿Œri©è?t4pÒ}tK?w£9Õ¤Þ?ši–ð½"ë?®¤Ycø?ïRÜâb?mS?¸¿´?cÚa¡ŒØm?EÕJ«e#?"0øLU¹³?k¤Ü'dœ-?ìRÄ¥ƒT*?¶ù­ü34
?{
ÄSI…²?q¡ß2/ö
?»¸þŠpB?¶Ëç	já?ïg'Ì@?5®løAi?`eç¡ Š`?nGé8iY/?'IŒˆÄ?ŒõN­)qÓ?íÔk£M]½?Å#T%ß?ƒ-J½º?'R\b'M¥?­íóFµÑF?›"ã\Â?îY8¦˜8N?‡,dÊ??rW:èýH?bÀ·
…Ïi?¨!Ž8Ev?†Cþfà¥@AGN4FGL J1431.5-6627?¾h"x~}À	‡Æ2~ØÀ:CÇE¤NÿÀ;±•ìeïH@äjÔ4J5@—dj㣩?Ï_T¹À«?Ì!^IŒf@BÌÛæED?öAkBS^?í:1…ý¿à¾Ý®‡¿èDƒBL"¿å"M!pèö¿ïÿò> w?å6YX`êUNASNone?äá%Ie¤ ?ÂTÄ^ªõ?ÞC'‡õ?"çTÄo´'?ÕA6{½À?ÂG8ßÖ¥û?âŽ"vÈg?Á)Ü¥æ?™U½x{NÆ?˜^^³~B?ÙNe¦7&?ÂÁíw߁þ?çÏg¸ºµã?­ºÔ®–Ìx?¢•ì³>}·?ì2Œ§ë,?ÌåðE‰?«Î±Ò–'"?å|Q+¹?§ûDQ»?¯¥üw/?Š'ÿ«¿\?Ñêfü
'?¦¯TÚ`?Þ•9bf?ÂÎfa4+?—Æê/•66?ŽÐ'ylÎ?à@}æ'!û?Â÷ÚJAuI?ÐÒ mÀš?Ýټ–Á?§^êGKE?¬Où•í7‡?æz¨f)n?ÄHˆk/41?àºÄ0ñå?²ö|hèã?²:Žo!©|?ý*ƒNc?Ùý"Ü_"6?²w‡@P¨?ÖoÖpÔBQ?°…ï"*?º*€KÌ}?Ÿ Ëß^l>?á'ľ5…H?°µkmàxéMIXED4FGL J1433.8-6357?îÉÐ"}6À
R˜˜—;À:áÍ:°ÕöÀ<§³Ó׃	@GpxŽ@¸îÿ&¼,?Ö×.Û4ă?ïÿ—?LF*@
φþŒby@6Ö)—Óò?îª÷?g?ïä;û…G?°1æA'òa¿çx!m
¿íñ܆~3ã¿ïÿ\‹/ôUNASNone?×ÝãZ­Ë€?»XÓx/?ÓÎlÒU?ÂTéJu³Ð?ÕN‹åb+?À8biy
?ºðè(%–›?¹øJ¿kæ-?Ô÷Çê1Y?dz—g$?â%ÿY0H?Æ¡*BÚ×?ä\H4½?²ÛIÐ4?ÃáÜó]?§­VƒÓa?Ë{ýSŸ±®?¬‹¸ú?É/?ÕBëk(?²öá<=?â£sh"£r?µGíÓ5OK?µØ¸UùN?|ñ7þ.?Ðxç	0w¹?¿½#T¡u?ÖÍ̽™D?Äx™6ûÈ@?عL95ù?Ã7v¾6ù?¬xÓ©Êd?²."σ¬
?Ô)Äé˜NZ?ÍD§S/kÂ?ä#PÎ,Q?ÌiçOZZ?Ý>§J‡7Â?µeýâA?Í)Òâ:5?²@"Î
®?Ô,oEnZb?²˜K"Æu[?ÄsL¼#åÁ?°ƒh9V68?æÇǔK'?¹\:$<k?Àm"ò¯¤7?­•F–ÅÝMMIXED4FGL J1436.4+3900?àèV$¤Ð@PG͉‹.À;¥á¨&$WÀ<ë]à…ç5@ `¾$ƒæ?ÿÓ¯tÍ1w?ÎÆCÜ"Ö?¡SÀúå?Ӟ¤Zè®Ö@3Ý	°Øпëkô0õk?ä(½ž†"X¿Ü³T€µÇø¿å†žEÑ¿Õ½ÄܓiT¿Ó±<MŽ(LUNASNone?ïÃ3+%ž?nî¶k1]b?F¹&á' ³?7\ѐ¼û¶?{E«LsÈ?mKá^U?ïÊü>~?u^6ª«¡™?FÜÖD0$/?OFû?mZ?w‡1¶©?srHú¸?ï[_㦔:?~‹¼¤	?bÀàÛ¤]?^TߖV*È?';çt´V
?|˜£*)±?ﮁEýÊ?c^%úalÄ?ZªM8õlb?E*n!Ës³?
e2ä?c	¾ÊÊvÙ?ïo[ó›Ä?"xxÜe"*?X7æòúö6?L¥/=`q=?ŠÖ¬ì+?ƒ1ÎN˜?ïdHN£Q(?–'¶ȹ?Y#zRâ¨?eµ7%¤^?'ä¾€åµÕ?•·`>X?î·A·Ò·?ç¦½¥"¸?lj­!{š¿?dÌ:´éwš?¢Å9±VÔ?&Ùñ¤¯?ïhɏwú?'ÓdEÐU?mraIƒ›?b-9±•üd?›DšŸåc?'ºià#Ú»AGN4FGL J1438.0+0219?ÀJó@;ã@K6-œñ<ïÀ;MÆF ÎAÀ<¦MÝÙe@4œ´V3h@Y¨Íê>?Ñö«XþÒ?ŊnÙQ•t?ïXBKÔê¨@¤–^PÃ<¿íN¶È¥ ?ï÷䨋¤ä¿ç‡âg^3¿áv"@Áç¿ä©Y?·P¿ïڅAÈÍ9UNASNone?ïë!'(I1?V	ÛÇv¬œ?>Á'¦-Ù?2Áþ6^æ?a¦²Îf?SƒCãÏÞ¨?ïÛâɌ?na€»3¯?AÑå6bT?J¶4°•\?o©zå‡ÚY?j'ß€?ï—ß"¬Äç?zôK"¡Y"?ZïûèN¡Ž?Y|ö¯Ý?†ªT­L?z%Æ }Ôb?ﺦE¾??[í9s{?`.÷ýæ"Ü?BzÙns4?z•a<º'O?Y§AìF?ïЁkü?iA‰×Á‡É?Liþj¹eG?A	Yáöî?t1÷à&ë?gcœ(á?~áÌ'?‡ý;'mÏh?Tß<kä%>?]ÁE&õ$?Š÷8´'—?†DA>ø?ï:¬>6òZ?‡hO÷C€Ï?fœ…Ðm¤÷?h3ÀuË9?•Öç'Û'
?†
½±‡?ïK¬Gµåï?wÃá}ö0b?p£ŽÍ$@ë?]ÎF®S?'a"Zõ Õ?vnCÉf7ƒAGN4FGL J1439.2-5142?ߤú©\Ó@ºø>jžÚÀ:"…fîÀ;¬ÿðÇô@ìüÝ5М@®}Vlô?ÐsÀA#6?È
‰Æ½¿?úRš×‡;?ýàwÇaÓÛ?¡g"@
ƒ™¿ç<ž_æð¿ã«4–àµ¿è«e©¨–¿ïÿúVrÓ\?Ó_o|9·\UNASNone?ájÌtÕ?ÄiŸÆÉö?"þå£4,?Šã©"*È??ܙHØÙAó?Äk¶e	ø…?ç	@Ó?Â
Ã{ÚÝ? k=RÖC?™æoÅ!R?϶å"Ì?À¹cHú›?è8ÉD×öL?­Ú%ª"l«?¤ð1æ2ø›?"`ÃÔSõ?ÉàÎr¥u+?«{›škJ?ééP,#…§?žÏ»ÉØ?œÜ".å_…?{`&®…?Ä¿,Ȃ\´?›®·¢"õ?ÔØ~+<f?ÀÝ7=Pe?œ£|áóÌ?'k$/B	{?䮥œùÿ?Áy»áJ»Ä?Ü*ŒçÀª;?Ê}‡Šxis?¯?ªæçÃ?¯öäƐ3?ßí}ÕK
?Ɋ"Kb¹?áÝv_¥#ˆ?²"¥›§Þ"?´öG*Zb? ~–Ï]øc?ׁv´¸?±•<q-;c?⚽õðÕ?¯C´©£$?©Uï¯Qœ?"@
6ó?ןÈ×t4?­$á= ‰MIXED4FGL J1441.4-1934¿ê" ½""@B¦µ(À:ñ"Nü½À<{Ó"Qc @!-"Pª<?õdãåFn?Õ3_¿-R?à
¨š¾\È@"•ƒŠcœ?ôùkjÏ?½|­_I<¿ç9äàõ?ؕAED­¯?°O\8û¿ÇRl´^@þ¿ïýʀÂ2?UNASNone?íA€èÀÐ?º(BzŠ?œ½'@e½ø?¸7	غÃ?­‰(Ñ8	?¦Åpqj+?îYO3'I`?¬ÁÚkâJ?"+å_`zÏ? §]@f¼? U†¯Œ?£G}&K?ìƖ\Ó³?¤$Ax§?¡¼–ŽkJù?–çNДúÆ?°íØ×£ê?ž¯!ÙÚ×?æþÌág?©þ­e@†	?˜Rmmé'ü?"yL̈́õ?Ð}?fi˜?©ÿ²;÷³ó?ìF¢¾RØâ?¶.dê=à†?ŸMü.²?«Á—áðM?¶£ºX À?°cå‹N­?ëwÝ©§â?ÀiÍח^´?®]:+•?·/ðůµ?µzçòa?°ù^Xku?ë
,ìÑ?¨äžú§\˜?¥£!ÿ?võ?š-Ùöÿ+?¼Ž™Ÿ}?¥/o%Á¡?ßÖõ0÷?·ÑN¹6ó?Ÿ'óäé¤?–÷t
Ž°?Þþ©Ì 4Ç?¸ cŽŒùAGN4FGL J1442.0+0732?Ñ0vY<v@L£ä`gHäÀ:݃¡àøÀ<o?v7"Â@2G?ڋ|@aÓÅ'j?Ð1¾"ùò?ÕGfÿ1?ÿ0	}WC´?ûQ0αÿ?ï¦ÿ]ꏿã°É–·g
¿á™î=µÃ¿ã–€À.Ù²¿ê_`—Ì:¿ïƽ FUNASNone?íóÇTŠ=S?¡9YêŒcA?‰…j†³BJ?}¤j:(îR?ªb0g(B?ž9wï˜?팊[oé?©D#¹v6q?¡ngzI?¡(Ž—Ž`?¥ÉEäÓ¹,?œ‰-T¿Å?í¸ä^—»?›Çè͹zÃ?–Þ–|B?€Pý†n"?©tx2?"âÄKm‡?êQñËp?–A†‹‰†]?µ¥½ä-Ñ?ø@ÕÑõ?ºwŠŒF±?ŽÊë‰Þ?êçr8	d`?±Ýa=FW^? É)6&¤ý?'dŠ
øv?À/ìÓc¥þ?°°´õ?éP¦-¦¬R?À–ÏZYŠ?¹Mß =`~?¸ˆô¯	°g?¼,ïrû0t?±zùY~?ësç¦Aó•?¦ëN®2?¤,(êd?"Úª!§ð?ºJ®WŸVÐ?¢LW˲µ8?âׇ֣=?¦&Q'¼xæ?ÅCeÔßڊ?¤¦ÊüvF?Ï^zБä€?£¼¬§ÀLAGN4FGL J1442.1-2800¿âs'ó@<ÌRş±âÀ:|غ@ÙÀ<A˜ý'gv@éN
'@cq|D=?Ƒf"ÄJr?×âûã:Í[@¶ˆ7q†U?öKÐc\0?ß¡—_,¶A¿Ýœ"`IÁÀ¿æ¤ªÚ3½¿î»CÝOÒ¿ïù~¿\¢¿îvª¡~ÀOUNASNone?èÃÔÉô^?ÂCËî´?¥@_Þ?ƒ?«N—©?Ç —ãi¤è?Àaz	l¡z?á3µ{;Ny?˺5:ÊVP?× ¼8*?ÉÒėê~?ºYÑ5Dãè?®Ï®¢–ø'?çDÓé?°Áv {r?»Š•3*7?¤FqqíÒ?ÅÕ¥ZåK@?©;Žjt9¤?à58	l÷`?¦îy¦Ò@?ÓÐ^…Oj?§ï³<'û?NJb͈<-?œV`KÿŽ¿?äÛóÚ®?ÆÇZ>‡F¨?²&·¯ò0?°RŸfæ}ž?Ó^œ	­Ë!?Åbz˚•?Ô,×"öt?ͤ*Z‹V?áV'o‹…?Ð*(vÛmh?ÂLü‰å?¸5BRg?âø¨ÂEN-?´PMbmå4?Äöª—?¬¿W[kš?Ï&²ã'é9?°­ìŸh?ÍÂåj?¥Ð`¹ªæ[?Ýñ6wúý&?´Iâ"~†A?Ó-¼€MÏ?®7'ýÍMIXED4FGL J1442.1-3707?ìxþS­|%@4­3;–¯À:ÏeóSIÀ<"­Ù©T@ 6šn*Õí?þ'Xœ‰8?ȁ'ºýíV?ÁmhxºPô?ù¿ë¨Z&½@\"H?ïëy@×æ¿âúò¿Ðû¿à¥lZþ¿×i#°q¿à™RÓº}¿æ±·û"pUNASNone?ïºìµ `]?pʓ7°ëx?Qµâ,‰æ"?Føkim?~,³ËŸª?nåžj|?ïgß:½?‰ÿâ܀4s?nxÅ`Š@?puUìÂrÃ?Ž‡[Ï?µü?†=ÿËïÜ?ïoœ£NW?xØÕp_?eX$MJK?hÞx¶U½?ŽÂò;Bâƒ?s¢OÂSUÌ?îˆùçô+È?{È^°9ñ?'/ ÏìXƒ?_©P£¶?¢äyM%æ?zxšíK?éðÂ?‰ùTöj–?d¡¨cc`"?Zû¼}5/?Šª›¨C?{ÿ|N9†Ð?înh±wåG?¢N£8?;É?€æ¡dµ%'?…B÷Ý?¤ß̐´:&?Ÿè¹Î~Žâ?îìáå¹?ˆñTÜõ:´?lïåïž4?d# Ï\	?žß!§ßFf?‡Q:CŒž?ëÞ¤´¤k?•j†Ħø?•üua‡?~ŠÜ^Ý}l?»‹Á»\ô?"×+0GAGN4FGL J1443.7-7037¿àUÓ):êjÀ#‡ãÑÌÀ:
j»_¼ÿÀ<¸{0œ@rôf¹@ó¢#«×?ÁDyA_ò?À?PøÀñw?ýò–³5L@ÙÌ¥	º>?ïáö?6÷Ž¿âÅõåÊË¿ä_²?¿à²üÁ‡¿è½/Á
ÑпïÿüoQÇsUNASNone3FGL J1444.0-7033?êéÝR<I?Á¦×o½þ?—¯?%ãG?¤5ûU?Áb¢Ñ?'?½
®òÏÉ_?éދr~;‰?¼ËìÔÕ?~tºù ùÜ?|N~àmd?ǒ,_PêÌ?¼6ó(£"¡?îbVŒÝ&??"´òµƒ?€½îÛ8ú?xP5y=ì?¥Ú'´g	Ö?'¦(Öàb[?íŒ!É©VÑ?€¡ÿÓd?'±¸º"‡?fÎØáE9L?®eU‹ þ*?~ŠÜ†¸õ?ät´±\?Ç5#Ã~še?±HÌ>àÐ
?­Fœ/kÀ}?ÒÅÁ†®Á…?Ãð½Sg?ä LÞw?É oÁÙԝ?X<fL?'¤IL´H?ÖõÞI¡à?ÈØޑMù;?ë!\>¢Û•?¨ÐŽ1i>?š@@aïß!?—m(ÿ&?À2†ù6•Ç?¥NVÐa?éS"Œš?—t5¹Ë°?§«Êw÷¢'?ƒý(ý9?Ä¿äyÎ?•"ðË«PAGN4FGL J1444.1+7601?È» ày—@C˜P%"õÀ;›Ãèø|~À<÷Â,_Ú@QRÖç'Ü@E]Ø"k?ÔZ^ï®?ËC扷N`?ï>~jê?þÅúˍ³¿î¨f»ö»´?ïüKuIX9¿ÔD­®úSï¿äÏBrì1¿ã1ÿ÷œ"0¿ïý³¥ÝuUNASNone?ï»Ó˜?o|¿‹\?_:hsÁJ?RÜßB³í?z—Ç÷áù?j/CY"ø@?ﺋhm@?z¯Âr¥<Ò?W`Kí°Ç?_§Ï?(ký?|ó³²ô°S?uI…/g"?ï0U[¸HÂ?†Ìþ²(c?yeбä47?z7ÄÇ­™¥?"›àUF¬­?'ka<?ïa|wð[?kŸl¯(š?xªÑ嶌?\r73­?‹K™Éy·û?eèÊî?ïoå,ÙÂ?'?˜#QX­?nŠ
4÷'?b"}¢wv ?Œ–A¯Ô—½?ͽ¡)2?ï,͹ð…?"ߥߦ'Ü?m·8$?vÔ'Ô?:Þ?–¯aݼå?Ñƒ¢°p?î"Deé–?"«éù'l?‡V'ç[‰ã?…ÎPT?¡æ%ߖ1?EsÃhø?î¨Îkïx…?…j6´ÚÙ#?'|"]ŽÐº?r3óSrŽ€? Óø(.î?'´2ùAGN4FGL J1444.8+3645?ä‹;¿…@P
·AJM+À;	5œ™ÿÀ<r@žUÀý@xi^hk#?üŠÉ‡î"?ä!j³Ó?è)¬¡´N@8³¥´Z@͓´RW'?ïh<>õ‰/¿éHQ¨i@5¿á¼ˆ¿îm¿íQ‡aˆ±¿ïí•Ïà}"¿ïøtP3ôúUNASNone?ìK"ÝG³?¸S$ú'+?€jìÎÄÅ?}‹ö5ÙX?»™'(á?·ˆáuoP—?쨢'mƒÅ?·¯œH9Í?ª7]ú14?°€—Á²z?«>¼†âˆ?¨§Ð?Ó<™?ì–÷'ê*?¥žt
²´â? ãÎܬ?"8<‡oËj?·V_JLÜ?¢t?sªT?é¢`å?Ã?§ºté0è?¯ÒY9éA? ÆÅlsU>?Áæ‡¨´?¢exbŽÖÍ?èù6ML—'?ÂP.û"ßè?™˜·†ƒn?"ÏO|ø §?ÈèÚyÄÎ?ÁÆ/ãÕ?ç¢^kUÜ?ÊO$DFÆ?ÁsÛàÍ
?ijLžPë?À«ý…"?º@wÏDv?éžúkäý?¯ƒ…"ÏÁy?¦,ÚXÊ?–f´T‡¡?ÃøßÉÃqÉ?«—¼}Qíç?äÒ­ç¯Q<?¸ì§Ëšú?­³‡KKHw?°"²| Ä?Ò¤3Gø^˜?¶¸åüÂAGN4FGL J1444.9-5939¿ìTۓRò?½Hô‹(À7à°.0"óÀ9Õ~;oA×@ס–¾@»œ=¸È3?»ZÀ?ö?×)±>y@ Vlô!?÷ɋúŸ™?î]/Ÿ¾w¿ÎIÊäÀ3Œ¿æä:og—¿ë^u×±ç¿ïÏk¾Td¿ï÷ú"‡UNASNone?ªW§Ù8Æ?²ˆãª9?åœÍ¡¢Á?ÍÄ;ÆL!Ž?ф'pf€¤?Ëá4Žæ?ˆÛ!9»¬w?–˜—ƒBSÝ?áÒiT
!?Ä5ꐵ¢í?ە#n'{?Ä, 7ÿ†ð?¸ydTÝ4Ë?©ãL`ÃÉ ?Úï"ÌqÌæ?¹Xšô–?Þò"oH?¸Åã"QšÁ?VSѳÆQm?=þÜ/
@?Ø´"eMÌ?ª›ÂÎ"5«?㚌d8?ªŸ´¡îãß?"ÿ¦í(ݦ?±}6¨ç?ç?ñ÷Ø?˽€å©Î¬?Ð0#k6|5?ÊrK»¯?v;K
¥'?®8ô^;?⺵Áÿz…?ÊÚj,¢(?Ú1§Oî2?Ê¿ÿ˜ë¸?°CÝò?£jHPù?Û»°×ñš?½ìöøoh?à«ôKR?½–ÝÁU?.Û&[¦EW?)jðwŽ²?ÞÚãwx?´ùNü±?àñ$Ûà¸?´†Ú—iMIXED4FGL J1447.4-5757¿ëj(1™Íh?ø^Ç»ëÓùÀ8‡¾[ðÁŸÀ:¼ÏJ«@j33fà@ký."h?·R‹íš<?ÜVômû†@û*ÂKi‹?ú"ŠÑ¹õ?ïõÄ"`¿ÓÏ© Z8¿æMOÿqº­¿ìzÆ:"‰¿ì¨õŒßvó¿ïþp]áÁUNASNone3FGL J1447.3-5800?w y~È
?zŋ¼–†°?í.­"ɕ?¸SVÙÊnö?¶‰0¢—?·VœE¥¹~?"‡{ 9?£Ú*íå?â¢
'9½?ÉâÎýå°?كÌMuÿŒ?É$ùÝYÀn?³;²Ñíö?£g_Ñ|†?äbä#w÷?´=Î:tÀÓ?Òkדiµ?²F‰'5Âè?‡ÜZæ(ß	?hH‰}`µ?áp&ºÔÓ?©Ú%1àR?ÜaÜy?©ÁÙx³™@?y^¤ú@x?u¸Ó	>¥}?ìvV6Ԏž?¸<[ <T?º·cüK7?·…We"Ø?'9Á$÷}õ?•ªEÑTø©?â0‡ò¸I?ÎÔjTKuŽ?Û
"†­?ÎÂÏJ""?¨s¹ç¶?tÛ
5T?æaºå;%?¶¦_!?Ð.øU;Ç?³Õçåií?bàhÜʈ/?IŽbûÃu?ãSö½›¾?³‹»²«i?Ù2Rî9"?³"|ɹ£ÎPSR4FGL J1449.8-5923c¿ï[U æ?·a» ™VíÀ8¨f±åÀºÀ:B†Î»ºV@¥{Ð'@jTà,%"?Á¾x÷¼Q?×Xö;[á@•!4y@¦ã™—ì¿Ý'ހÔPп£TcÀªæ¯¿ÜßLÁ¤¥'¿éFÝÕ2ÌÜ¿íÏr™{¿ïþ€£ÿN)UNASNone$?ž"h/ Hä?—l¾7?³‡§ï©¸Ï?°ÁL¯{Æ.?ì÷ÀIo?²†\Qˆ?©¦@7{âç?ªö§dþõ?¿&êÔ¹o?±)ëâ–×€?ꀾ¢O??¶AÕèsT2?´¬ìP®k?¡˜ª&×ÿ?ËìdÕöÞ?°DÁ?Ÿ?æƒq,Ï'+?²6±q?¦'l÷,?ˆ3gß­è?·}Ôô¼ê|?"ûšÌ'Áó?ë¨'²çÁ?šU±s'-v?'>ÛÑÛ&?ˆOèy[I?ºßèÃ?¶AG?ì c'?·
£Ÿµp?—#ˆÅV?˜Ƹ@
Î?¿1>o"W?µóÓIÇ&ù?ë`»ñՒ;?¶ê7kÒ%?©ÈQP™d?–Fʏ'Ë?Ëú`
±Ä^?´¸¹²i‡?çdß'Ã='?µßQÕLÞ?ˆ=.
ùJ¬?qíc8;2??½!deü?£,9vœ©?ëúÞƇÕ?¤çc í©OTHER4FGL J1450.8-1424¿ã3Ô7œ›Ï@C®Ûʖ'À:ñ9>/HÀ<«©Ìíƒü@¦o;÷ýÓ?ÿ	‡ƒ U?ËzÆ[¯S?àšIÂÁ±@b.ä¬?ýZæØñ~?ïÿ•!îZ¿ß°nh@†¿Ðä¶Î]Ç¿àd"‰—Ã׿ïÿþó…õ¿í<¢¤@UNASNone?êÞN¡Æ?¿fP	5fr?¼Ç(%ÁŽ3?¹L³=jÕÈ?²¹åbœŒ¦?¬ñbQ…Ž?âçÔîŒî™?ÇÛE,ý0?Ó¶²5¿!
?Æ"–lµØ?¹æ°P"?®*ñIœ¢?äê©ÂÉn?³‰ß"3t?Ë+¢61{‰?°0rM¸54?Á)¶Á·^À?¦j²z÷Ù?ãêh,þÕ?¤®É	g?ϽÐkÎìH?¤Êæ"~iÁ?Â
…ñWVå?•¬n]€¹¤?ç]̚*–µ?À«ëÃTup?óÜ1}H?¼ÜyŠ|é?½©ã
HOÇ?±ÂÕHø?ס¼ÜGr?É®Nñ÷1?ߏ
Òõc?̄H>]3?óžp¡†V?µ*ng·€R?à³sx{?¸ví&ù?ÓTà UyÉ?¶Þ˜DЁ?Ɗy‡*?®XvÅ/?Չ"lÒê?«'í PÑ?٘®1ס?²ÕdT›ì?Ðݽbu?¨ˆþț°bMIXED4FGL J1451.6-3726?ÙäԊAþ@3‰ ÝDÀ:†\ø(›*À<*ÐíýZ@Ÿ¹"uö§@ž¢ûB+?ΏbÞòi?Ø}VÂÚZª@'!ý€É¿@~AÉùÞ©?î¼´áɉ ?ëmô?,­¿ÚLǤùv¿è<¦ÿ³©æ¿á+þöë"H¿ðUNASNone?î¹b©(¿?•'©½šÅ?‡né"D^?'
sðås?%¾åàBk?È£r`o¬?ì"Ïéjoé?µ¥%Yyð'?­¶–#Ÿ?Á?°UH7b~?©kDó±?¤Hä–à/??íð'3º[? )ZTO܎? H¨W{'?'ÒåæZYÁ?­ØTúµ¹?˜Æ)TT]?és-s£N? SÕuTû6?¸oáòÑ?™uÒ®ÒՔ?»ö³P$Â?˜{Z)šÊ?í2/ÐR=e?§6Ø#u5?ž-ÏÓÌ?˜ýÅ͆…?­ÓìÀÒ? ªÙÄOI?çYيËJ—?Æ7—2®uk?Ĉ<Ã"·?ÂÑZ#µ¢?¼ ºKâ?²ƒ´³?êbÉZÉǁ?«AŠým?­Ñ,š3X?œîìü$û£?¾ÛYÏÌ?¥ƒõšgò?á7º
A;M?°ÐÉè?Ê2«¬tEU?±ÐL:—Ï?Ðw6Cf»?®ååY'õ‹AGN4FGL J1452.0-4148?㳘àOû/@/J^±¬À;$üȼÀ<ƒ|Æúû´@ Êì=ÖOX?ÿ´W£U?Çú–È¿\…;T%Ï?™ÿÑån@T$Ñp |?¾=‰ÎJ{N¿áû¶úÓpU¿Ú׶_Íðä¿ÜsÿÁ–¸¿¿Ý<ñ¢ðŠ¿ðUNASNone?ïÀ)ß³•?s9%X†¬?LüÜoF?@5w²¦$.?|Kt Kq'?qÜ«¼&ü?ï¢"ò? RÝ]?d"Jþ퍍?lK	"ÆÌ?™Ù&H$Œ?žú¿ï?ïKà£Ä?à?ƒ÷‹TÔ?dUϵöJ?e¼D3¢L?"ùI
­@)?'öN©ð{?î󊇔¹?yB?ÒÀ7+?f¶ùMt­?IÕgo+?ž·ÏÞ¦É@?yoÀîw`l?ï•ú¸9å ?'Š"2šd?V4+6×°ë?L'`‹ae?‡ºÌ'»Ñ?I'EO#®?íã$́è?²¬•µÚç?qx\UëíÃ?é/Ðóc?¯ž§¯ã±6?²3³Ïo«?LbY<?Õ·º¾m¿?kr…-þÍD?e3 4/ã?£/bè.\r?S:J彛?ììþŠ×V`?"©'ǓSº?|0.\?h£¡ÍÑú?¶Õ'nR?• Êi´éAGN4FGL J1454.3-5551?å½Åo$>è@äI:ÜtàÀ9ö¢ñ10$À;Xù"«ô@"£ÊŸöÖ@zh˜q?ф}*[?Þ|´†"éß@Œûü@_œ"JÐ3?î…ëÃ¹ÿ?°Ý§Û¦¯¿êóæasbx¿éÙ—â¿ë
´Û¿¿ïýf],+UNASNone?æjqsF?Ĩ'ÀB‹ý?°ÿ›üiUV?­"©*<[Ô?Í×ô;YP?ÂJ%RŸà?àžNoNÂ[?É#ÖmFø?¹ˆž"Œ6?±dê2Ie?ØÀùô'ý?Æûõj‹ö?⪾ª¶È?³*óÎJN£?¸|"Ð,å?¢êÇ>Ûl?ԋ]w–w?²yQÕ;¯y?ß݆É2c€?£8¶ÂÙµ½?Æl¤/Âí?ž ÀR¶žG?Ôì'ÿyÈ?¡@Ój+à?ÚÁº.(v0?ÂêÕ@¹®?Ê®°—Œùù?À"™'OâÛ?×æí†Ô?ÃA̸Ït?Ìð"AÀ?Åýt~Eð?Ë\m«Ìnz?Ãþ­ ó¼6?â$¨t"ñ?Ê^Fàî?Ô¨pâkD?³0'ƒF?Ä\®¨Z¸Ä?¯v|xœ?à"›ä³¯?·ÆK›NX?É<Ó×]ç?¡ÏV)'?Òþ=_So
?¯`¬ ÜxÏ?à1¬[á`?¬×¸"MÝÖMIXED4FGL J1454.3-3946?ìX½ß
@1<¯bk/À:ϳô¬æÀ<̙¡&@ýˆf# @ÿMzÝð?Ûô°@¥¾?ß?p\‰?ø)&i÷@´^»!S¸?ä»!©ô¿éî4Ïëe¿ãç ÏÃÍ¿ïÿÿ>¹ú?ïÿ‰ñÇ®?ã–!‰"UNASNone?ïªgû'?ŠÙ(zÈs?eô€j%'&?q8²Ï¤±8?÷4ð®?…®úîŒÿÇ?îV~M'?¶‡ *7?jywc"w?›WŽì¸?¦_ùºÁ‡t?³Ñ…ß?ì{²÷ʸ‡?£T·G—}¼?£)‰õ¹_p?–ÐO€ÃÜ?²£F͌?ƒ¬E¹_Â?ï©¢í G?xo²'²_?0àùX9?1+§ãõ?…ý«8"Ê?x>—Zô?îôw Gô
?¡-p^z?…ƒ×
tjd?‡¨
¢¹€?–¯0vî³w?œ´áÝ?ì]•t¶?"–á"–6?¡ãÙæg?´±ð²Âûâ?´!k/z7?ºUê5q¬?é¹pÄ/¼©?ªií¸ã]s?±C¬¼±Ù? {Ÿ'ÝT?À›‡¡±?£ñ0
Ì·Í?î<:²:?¥Ä¯¡S?WŠŠ9¬­s?bóAÏñ)?®èΰl?¥rFù‹0AGN4FGL J1456.3-5419?ﮜcVE@ي¨exÀ:Symª'†À;Ôj:0}v@Ið<h'@ž˜ÜÛ7Ê?ËOž"ë<?Ú6=©¯@}¦Z?þ)Þb÷F?êQMÀR@¿çœ'0>Œ-¿á>ƒö¿æ¡o† ˜'¿í«a·€	¿ïý\á0UNASNone?Ú¦uÂqK"?Àusg´L×?ÆhöÙ»¥?´Þ°Ñ?Ú%аå™?À59aV?ԜúÀÐë?œ:¢'S?Ä_‹Uß³?·"Àüœä¡?àš-'Ö^?Ác[=­#~?à´íM~kž?³>'h¯Ôµ?Ááeˆùkð?¥¡ôgî?Õ¥r †rË?±ºté2Ÿ?Ø£uh5?¥Y‰?о_EN­|?¤¶'À	æv?֞++IQO?ªŒ4"!ٛ?Î2wÔR?·OgûM?ÒWÓûY?¾o ?ÒÌ?ގðx£Ì?ÀփSuâŸ?½*Ô?ûó?·`£ÿ…#?Î2ô$¿<?ȳ 
i?äÍèo"a?Ã×ÃÕ´?ՆqB¨?²¢ýQ)1_?É#€i-&e?¯1ÿÎÏ'è?ÝçÎÆL*%?µ©ìuè4?À ž	"§ß?š¶×B¶²?؄¢®"ô?´1~·[›?ßkK7^?´ Ó¸öYMIXED4FGL J1456.4-7129?dú» :)ÀÀ&`®–À:ðª¦1W'À<m¡â=wZ@m®˜YR­?ÿ¶JêßÝ?Òk–|ÚÑ?ØEAþ}@pë?~›@uVSsÅu¿ïýРkð¿?ïÿ¶~¬®I¿âå{ð;g¿Ùó:à%Å¿êmbnŠ!W¿ïþÇ1¾UNASNone?ì¤`±èè.?´Àšº	?Žã5zmý?Ž4ß{h:®?·"ΩpÒ?±÷þˆ>yú?í°;"€«?±œ¤f×C?†¢2$?™¼†?¯xDŽ"Å?°U
^jÓå?ìÔ7†_U?£_ÅòÄ×V?–‰vïr*?Ã©К´?³Ö¡píAÑ? ÉoŸ^Ð?ì4¬š»?‹ñ{GÃ?¡N[ü¬Ã«?|³€##'?²ï,ª»Ï?‡¤Zï@À?êp'¸ÆI?»¿/2ü	?›fý˜¥0"?•ÙÒDž?Äa^@õ`?¸åí†rù±?ê²dZ˜Ó?ÂÐö¿›?Ÿ¦ÈC_­
?§¶}ZS?ÁA–÷Ž?ÁXì
Í?ê	mëÁ?®±Mš†ŒH?¢"Å?"©‹ÏãtÝ?ÃXPÓ,7?«ò¿ò+±?èv0À´‡ÿ?¡æˆàŽËŠ?¯äÂ+Æó¾?"çË'qŽ,?Æ.q—5Ö? 55KNMAGN4FGL J1456.7-6050c¿îrH1ûƒL¿ùqÕëYÎÀ;e߅65FÀ<1vßZn@&£¨žð?ó­Â*²[1?Ê+?Éą¿¾Þ㥬Lz?öy^«‡ç@Êò4:o=¿ïÖHaÇó?ïí,•<=¿ì÷³•Ä"¿êzàñÇÙ?·4£ ®Œ¿Û­ë=ÑUNASNone3FGL J1456.7-6046 ?Îïôw¿1â?Ë÷Ͳ?Pã‡-8?SXQG<ÌÜ?è;'('¤?ËwÃþ?¾X¥ŒÛ´á?ŏÈ0A!š?*¡ßÑEß?œ?;~Tp?볖?œøõ?Ŝ6Çò?åNk:&Ã?²ÿþ;½lô?R¹ïþÈ?`ý,ÑC?ÔåÞ¤™/š?²þ¹s"M?ßÙ^ržzv?ıü&žü?{…ðŧv?zÉÚ)Û´Z?ߺWu˜ïŒ?Ä󠩶ÐÀ?є7r»'ð?ÊD67¥?f7܃ڰ²?f—é*Msã?ç¬i?ÊPð{0V?µ'«—Ó=?½
ÕÌ?ˆôwehð?¤ñ¾M÷èV?ìéú^ø«D?¾‰n†ÎïD?äv]:â³?±Ÿ{ʕ~Ç?WÜGڃE?‡N ̽Õ?Ö(†ïlÁ?±d³ÄD½?ÇÖX«'V?À®ø®Á¹?Žì¾ÕtXp?¡*R²}?鎶Ú@¨?Â}wˤ¿ÏMIXED4FGL J1458.8-2120?è°+†QÏ@@H‰ÁµA–À:eJýTTÀ<Ê8Ö?@ªqùílU?üäœ,ý?Ä·.jv–_?Ûë<äâÃ.@à8ýw"@p^ùÞ?ú¢É¿eQÃÂ)"¿É|ƺš¿ãÕô~A¤e¿ë6zæP+'¿ëü?¶Ï4†UNASNone3FGL J1458.7-2120?ØÝô'Ïî?Âú‰Òöã?á9¶+íæð?ÄóAˆ$k?²º~¥¡Ç?¨›?ñcƒ?áìŸÉ,?Ç×+ò€
?ÕãÕ/¥g·?Æúk/g»?¹²ÈŒÈ?§õ}†m¶Ê?ÔºC±
\=?´^v]ù\,?á÷yÊ$ž?¶)ù™¶"?½["êªr?¤'ŠAóüx?æÅ{ß
Zö? dh=â?ÇØîKÖå?(†ÐÌÞ+?º"Doèè"?Âú~|V?ÎV7žkª7?¼¸ZÉ­¼?å^»ì;?·gy¥¢*?¸]±^wÓ£?­÷9®ˆ¥<?Ôø¤Ä‰¸?È	©È¢?á iù¿Ê?Ê7pΖ?Áoõíi?³'Ã3¡6?ŅXËYkg?°¢±¤Hl?ç:åVÜ?¶…Ë@²?¼C~""rN?§§»u€m?à‡x@Ó?«Àz¯á"?Ó
Sòè·±?¬úZâj<?Éã:9.AS?¢Hú
kÀxMIXED4FGL J1500.1-5846?´ Á÷T?¶j#¤
ÖÀ8®n‰J—À:'¤ÑÜF@¶ßªõâp@7րªµK?ËØF=&&/?ÈL«êªr?þ¦îœ*m'@%ýžü¯é¿ë¶D•[Fx?ì_>Sù¿è2í"ñÚ¿é¹Õ䣃'¿ê1y¿ß~€¿á´¬¯öÓ1UNASNone	?Í<¥¢¼?À1'&=4?´‹t¹v"î?µJyÌÀL?æ&ÐY§Ä³?Äü9´2?²Y5ég?´y#¬d?±¨´ÏáòQ?¯¥Tõ¼	z?ë·¶F?¹9¶ðl?¿Cß¹õ•Õ?§H"­f-?×	wßé?°¦¬¬º?ç1ÁªÉ†‹?²¡"'x©d?Á‹[=hk?™/§íÌ?°,:®D?XSv?é7¨Ó=?'MAg®"?·#¿Ü§Ë?¬?Š,ã?®‰¸{0œ?²oÒ¹NT?ë3`8‹?¹Ï‡´Œ0?§œPƒ%8õ?¦3`¥Çó?¼'êÿà?¾òÏ!Þœ?ëWÚm°n?À6ùïÎ79?µ¿s¤2<?Ÿ4d»µ[?Ä\ÄÔ'V~?±­ðx)…«?è0ÜÜò*?²õÎ]LŠ"?¥Ã‡:¿¯?‰äKÚ¼'?´¹KÔyO?žª-ÊðR?ìž´™‹? !éM¥¿OTHER4FGL J1500.2+2640¿ÍºŒ';@N®"î9.À:ìðó®À=á{°z‡@ï¿ÿ^ðP@^@ÈG,?̈ѠF1?ïÿöàœj@Ú­æW¸N?þ äßh/ê?ïàÇ ½û#?ÖLòãÕ¨¿äáƒÞFqÔ¿îö'"׿ïö4osUb?ÃVú£ӀUNASNone?Ó976։m?ÉÍâ×%@V?ä×úˆíÇ?Ëh«vLÌ?¨¶ÇŒØ&?°«b™Ó%?®èD7·?³üÊ?ìTZ\Dx?¸œ½y«d3?«ÑÌöD=½?¦ÀeL•Aâ?ا‡g³8?³Ú¢œ§õ?Ú ¤³±¦^?³ö$`µâ?Éo§É™LÔ?®g=]Ðâþ?²}o€63R?˜Mƒ˜?í€2ê•?œg–'¤R¾?"Z;«ià?ƒ{3ƌ²?ÏW)6¸¬?ÅÃÇøIÏ?æúø\V?ÈM0•Ò˜?°jíåŸw?¯ññ^ýfs? ø2Ç¡–?°×Ë:æ"?í\Û¥O&Ñ?¸:à ¡"?©¡MxEñX?¨³>~é[?ÓÁޝÀÖÛ?²¿å»Ì˜v?Üx¾ Â¶Q?µíaw¤Q?ϊłøå§?²°>Š?ˆt£4æÛ?{}Š?ï=µjŸ?mæz'Y	?'^
"w¢¢?‡iUÝkÑ@PSR4FGL J1501.0-6310e¿î¾6ÃÀ Oœ'rÀ8AðáyÀ:c7ݼß@:<§P;'@¾¡žJÙB?¹ÑÓFäjù?Ò(ÝÚ;JY@Âl~®[È@ؐ$zß?ïÿA>8ÊÍ¿àzjÊy5v¿Þľ`xe¿ç§(bõ˜ž¿äQ¬šþ¿ïþi'O¦UNASNone3FGL J1457.6-6249 ?±ø©«Õé?¨þv{Ò÷C?¶¢ÆE?µŒâ¼
MZ?êì'Á?º ±Ü0Ã?Ѝ¾o?Źš‹1!
?È:1:pÐ?¿Pí ‡èu?áúª"yÛI?ð£XV¥¡?É
_P-Ñ?­S=˜%¡?Ï#£›w?°z¸!ÿ?áôˆC—À?²¿Å¿ß Ü?¿<˯¸·9?¥åY=at	?±'AÂ¥Óû?—µ0öXg?éèQÏ«y?¯Â€H³Ï°?ªSŠvÔP?¢Ÿ¶7`Ê?¶ŽÚz"®"?µƒêÑʬo?ëˆì	îÉ?¸Äƒ³®aµ?¹ñ:nªœe?¹õV…¦P?Ì©Îc-s?Ä÷¹Ï2ò_?å—eÕÜ7?Å÷ˆ'pO?ÀÙۑiR?§ŠÒ§8[?Î/à­Õ:Ú?±?Ê>쾞?ä=ï¦ìh?³´®9b?©s'^^y?—²ÔµÏ_?³sÄíŸ?£yÓ®>?ì˜wI|e?­éé{ÓWOTHER4FGL J1501.6-5236¿²•3$yïÌ@g¥ßøù|À:fž—/\À;Š]«¬Á•@®šǦ@ßæՌŽï?Õ/`àëgÃ?ãwÛÈgã@{6½+o?ú"1Ó·¢™?ÆÛ˜ÜZ^?èSðlõÍ¿åõJÖ½ç¿îˆÍ¿ì³ß@ñ^¿ïýZØ®UNASNone	?Ý&5éñ˵?Æ5 M	j"?¥,ÈPŠ^?¢.ÍWh?à¢>Ž`?ÆþëÐ?•?ÐQ>él7-?ÄWvƒî?ÎîáOn?Âށô?àO¥QŽ?Á:˜b¬?Þ
-Õ?%ô?²»üíÕD»?º]÷vĂ?¢ž"ˆi?Û^'íö	©?²"ÊÉȶ?Ì-c™­f?nŠPÊ?×GæÄÊ×?ª.qâ®Q?Ú¡Ž
^v?¦"ÆG¬ÏÈ?ǯ
¶ÄD5?»É¼Ko?´,+9y$W?¯Óúh'cë?玷+-ˆØ?ÀíTCp'?¶%ö-Ë®?´õ‰…?Õ§=´ÉÿF?É-?ÿƒ¤?âg¢_ª¤H?ƛbº'ì	?ÑÈ ‹÷Ö¢?°
FżV?Áãú_pí˜?¨ÞÓú,p?â¢ñ"'ÙI?³ÅüaÛR?±]§¼L@?Â&¹N×?Û%!Þ³:?µ7¼µÌÙ?àJ¸w¢›B?³×GÐfCÞMIXED4FGL J1502.2-5933¿ªâ4&úË¿è×z:XÁbÀ:6›X¶z{À<nšèN3@ìÖæ(ß@yn‡PÂ?Ó|_…?ïêÇß}( @·zâm©@÷½Ñ²9Ï¿ïò¶kawê?ïû|ã€m¿Ü‰¦qï0¥¿á?ÅGMƒ¿íûª€qªg¿èÃà•®UNASNone?¸|£ö^?¬ñF¼˜p?ÑYՄ€.?ÀjÝêá$?äC€¿aî?ÁÆ5×°ß?§|!T1²4?­±ö]š?ÚPé–Jô_?ÇV0ê"Å?á_ɲç?ŦäàÎU?Ò½c2]?°>–(¸ëJ?Õü)›Á÷?±‰È`‹?×FFT'ìk?±ð'×a	?ÀÐÀÕÑ5ñ?¢FRíG?朖
ØÑ?°ýdæ¯X?ļæÿí¥N?©(8Ëv×?¦ùdy_?¤þÃ@¼F?ѹØXû?ÁdtJ?æ2ÐYA?ÁéVÄ—€?'º:4?ˆè?š€ÔÂ2Â?ÜÚèß'q?ÌÌÑOÆ×?ṿ00?ÌF›Ð??Åd±G,±±?§
ÝkÞþÜ?Û3¨Õ\úh?¶±¦;¬A?Úþ‡¬¿?´â¸b?¡''Jb'?¶ùV³?é¨QݵË?´YÅÒFY7?Å׬µÍ?²žèџ¡MIXED4FGL J1502.6+0207?ïø¢áõ[•@Hï? §?uÀ;P¤J̓¬À<œ—w€j@ V"‰Š,ê?þ'ê–o ?ÐùùJ÷?ÃígaŽx?óy¡â=wZ?üjÔ²t[ò¿ïù™~Á¦ÿ?ïÕɕà§u?ï(¥:·‹ó¿åêa2Iÿ¿ÝŽè%Bڛ¿äƒÎSŒðUNASNone?ï͎"?'5†FA%?V Á«¯dh?'ÎýÏQ
?sÁ*Ōû?n•xâé¾{?ï®êKÇÿ?ïß'Õx?]³oþƒÏ?g´p¼Sù?€ŽÿKóÎ?{Ô
¤¸Íb?ï4š.á?ˆN'Z€â»?q™vp¹h?w­õÐ]ò@?•\ŽÁçP?"­ôèëT?î˜äþÐ]¯?ˆêU¡mê?÷?ìÆé'?tºq[ZY?¢rÈ×c?"æ˜4pžC?ïµ;`©8?vÛ´ÓÓ'?V²P ái?N·ºÎMŠ?µ»–Í#?tÝot¾"?ït@ĖG?ŸŒÿðJ1?s?˜¦:u÷?˜ìÊý}?š¡'¼~Á"?™‰sñ9IÀ?î­d&E9?':­Eµü-?wZ$ç´Ô?vŽÜ(Ø@?¢Cµ:ΡÓ?ŽÌ,v¨_?í(à¿Ô?¡öç**§È?…Ò|¿7E¹?…2¹ö_€?³þªož¬%? ¤a~ãqAGN4FGL J1504.6+4343¿Ô™~aûã@MAtNƒÀ;±ôr{HÀ<æ¦qq@!:¾lâ¬?ûBr5§º?Þ%€W©4A?Á°ûàá'?ß¼[»g @^"'GA³?íîÃA³©¿ëZ=c7ݽ¿é•¢:Å?¹yÿöDëB¿é™RÀ—¿Ò½å=ÜÚaUNASNone?ïÃܯÿô?wÍ`7ª?Rq;ä€?Hê®
'?yú5Pê2?uí@qŸ~…?ïz¢¬yƒ?'Nk=¨¼?dgEö
´?o:!À©Ý?Œ=ƒn4(?Rðùãí?ï*ÞÁ?‹Ê`™š[¼?iñõ¸ÂÁi?p²׳þ?™\oEãÂ?ŠZè:ޖ?ïFÀlê¯?xz'In3?eëÞ{o
ß?UŒÓ®?"jv¤Âc?wz¡1ï‹q?ïZ#°ð^‰?ŽÊÿŒ…?fÂVô÷N?b2™àZV	?'ã?½š?ŒÞ¶{žÿ,?îÚp\?¡T±%\i?m9<¿%}¿?{¶•ð™
? ‹E6¦ã? _3ò­?î@¡Æ8Þï?–8îc>v…?q-l«Â ?qEA¥×2‰?©Ð6
ijœ?•Páµ`KO?íÃi 5H?˜oq›Üf‰?uD	G'?t9¢)µV÷?°ÄoµA?—ÿmUeY˜AGN4FGL J1505.1-5145¿êQDóœfË@WbØ<l˜À:P•,L%À;'(mÝS-@A—ȉG@R.»Õ-Ä?×ìe$?ãrl™†Nc@Æ.Z†^S?ý«è¨ˆË¿ä"œ!´/È¿ã)¨¥¦V¿â³CÕAæ¿ê…AÁÇ¿éèv¬.ǔ¿ïÎ0»"¦UNASNone?¸¥Zˆéq?«d†-ÕF?›tS:¼&?'ÄÙµÔ½Ñ?ì¹ü‰Ð?¯mWÔú¯
?ݕ'fÒû?ÄͱT²p?¸i)±
?²¢-T	ç?ÜP¡,#ä%?Á±5³|Tö?ݤ=øð'?°Ø"-'c?¹|M쥍Ì?¡Áãq¡Oh?Ûü®‹]­?±ÖÉf@?×£}óö²N?­¸þ\éoX?°'F|Ñ?'ÏòìÓÆ?âN½'hO?°*'E_‰?¢Ô†þ3?•s}^Ù(? LÝ<&cü?—¨ïDh\,?íÚdë<#?¢yM]{½?ÉO…ZTW?ÁX
Òí?ÆË1ñX?Á¦L3ÎþD?ãùRz(î"?Ä+|Âý?Ò3´.è˜?¯O·zå€K?ÁQcŒŽ»'?¨ ?ÅП¹?âœ
BÄÜÐ?²k©]ÿ1?ÃN/ÔÀv?¥µéëÈcÒ?°K7ô?ž&wií$H?é#
'I´Ä?¬â
PÚƲMIXED4FGL J1505.3-5852?â·:I°€Ä¿Ø#dn•À8\ëÉVjÀ:ïLS•©@ÊþOPË@l»Ý'@/?ÐLÌamb?Ú@Z£'®@ Ÿ°4?ùB)Æ"¿Ù¼sƒ…[¿éyq%Ú¿æµ^ñýÞ¾¿æ~˜÷³*d¿íú'
‹þ¿ä8*lUNASNone? 	Ì2xA=?œ§s0€#Ç?~NšIoC0?…]€W¶ò±?îÂÆbz? *€—v?µÎ2 »@Æ?³ëÚŒ‡?¼±~þà¹?°­Q;VÏ7?é°	Ü]õ?¸ÓÏJ€'?¿ï"ÕÒÚ?¦8>‡e"£?¿™CüaÃr?¦Õ+CF»?èæåÒ­7?®‹†"´;?Ÿhqýu"?ˆµwE±»?­C·ãý-!?—9º›MÍ?í0€ò~A? $¶ž±2G?‹˜?>œ?ƒdLnbE/?€3éÚVO¦?}Ć3‹Ÿ½?ïPÏ\/g?ŒÅWƒ6»/?¡êŠïO7?¢êÈvè?Àì˃)HV?º$£–{4²?ê¦$p2ÿ?º8Ákßeð?·˜Í=yC? Ý¼(!Í©?¾€—a}k?¦Òá¥&3©?éJ9°ÙZ?¬Ü7Í3À?"ÆV&àç?t¯ŒCž|	?®
ˆ8+<? «í €3Y?íÌ?ik˜?¢–¤[daOTHER4FGL J1506.5-5708?ï÷døö?𻦺Œ¥À9*#²Œ¯¦À:ÈÃB	Ì@ƒÇaÓڈ@@ÝûÉ9š?ÑP¸_˜1?ÔÄÃÿž±@FGwÖ@°s#Ž$›?íçòpËD¿ßÁ‹›T.Ö¿äD8¿HB¿âë7@¿ì*í+&¿ïÿ·`)
UNASNone?·hƒõËý"?°é†ìUħ?›ÚͶXv?–'Òºrc<?ì4âæŒ?³SL6Ⱥ?Ðgýø
_¢?Æ7yØm?©®šæó*?¡°o7àý?æ1 zZl?Ǝê&f'?ҍȏIR?±¦ª÷€x¸?Ä~½ªðÙò?«(TçEÆt?á™lM¹¤Ú?² ÃˆW1R?ÑKÍ
+ÊV?©Pßú"±¶?¬ž•ȝ?Žxµx'D?å0)='?­!E‡å
]?­Ë¦¸	H?¢d>É~ ?µœ"…‹E?•/ðÕâím?í5˜°2Ö?§êKuÛ`?»e¢öSr³?·W}/«?­Æå@ÜË?¯+σä»&?ê¶ÝLÕNY?¼«
ZKû×?Ձ­i°?§Mmß"5?ěw"™?¬<*vÍÇ?åu¯áR?±яÚG?¿ ¹j``?¢gïd'«Þ?­hdQë?™e«ýà›*?êJ·wŒ9Æ?©qnˆBOTHER4FGL J1507.1-1901¿î)ôtþÑú@@©º^5?}À:Àh®?CÀ<)Táä·@ê+ÌâqO@œÃB	Ì?ÊK‰@[￲fCUë?è8)Âq)8@›oðRãÓ?í-$%y6M¿ê"`Ø\ù¿ì>â=ø¿Ä`‡êš"¿ïé¥J§Ãÿ¿Àø\È_UNASNone?ïÑâe1Õ]?qóû3kS?d´g&[¸?c8L‰…Ï1?ii3'³Øñ?i)žSLŒ*?H[RP?¢Q6È?q-k
¡'?éªLF	?‡O×1>aF?ƒ ˟¡«—?îªá"Zo?'F¹-û¿=?Ûˆ;Ÿ%?Ê'ÝÒw? Û'€èìÀ?VÁþs«!?ïŠ\S#NË?tí¸
Ž€?j1%£
òÃ?X8àXß,?†Ü¡ÉAf£?rS(r@a?ïxß'Rˆ?ŽOñw)–Í?ÈTÙP\Ç?ƒHÒ¹Ä/?ÿÍK"úc?'é¾_u«.?îÑÛ¢R¥¿?£#¨¶ùîò?/¡ÑŸ?"Jí¯¥?ø£F>ôJ?›6o¬ý?íVnãHË?Ÿ5˜	Ãð}?h«ñþ
?‹š…¬ñä?±'ú]
S#?šIáµá?îZúѱ§Ç?—f€£º•ú?‹g°Á½õÐ?"z;Nms?£vfµQí?•*Èð8%¥AGN4FGL J1507.9-6228e¿è¡Ktü	À
@$ À8èO,ý"À;`CނØ@"`¼x{?û÷Oݍå0?°h­é\Ð?Uö´9És~?îz£q+3?îã!øÎ2¿ÂM%²—¿àWÕ©ë u¿Ú~½ÀjhÔ¿ÖCÐú®ÝN¿Ó"j@ºˆUNASNone3FGL J1506.6-6219?ᦇú(?Ê	Îy¹ï?k®j%Û?bèz4qõ,?Ü=nrŠ??Ê&ðjòÎ?ÙӐ«‰[3?ÊêûEÇ?™ö%Rù5Ü?÷XIiÁÀ?âF†5•8?Ê@ɂÚ)F?àÒ˜ýx¢?´^˜?—Ü]b?'çwÚkÏ?ÜÜ´ü¡{»?³êðS¤ù?Õ­ï%Á?­ÅÓüofe?´ñ$XŁ?—ò@h¾?âŠãâyB?®FÜ)Ùd­?×Bnz+h?Ȭõ ?ƒÙo&ç;? †š-P5Ç?äc¬äÇ?ÈÚT—(r‡?Åü—Ï®Ã;?Ã?U"°˜(?¡|±lÒ?°ÅI-*–?éióý'?Ãسå%÷?ÖǺ D:?¶Fé—ŒŠ?RŽyGB?•;㿂Œ?㱎{êmX?¶%Š€C~§?Ã6¹=¡?§®—8³~1?¼Ç2p¸?§ö×7^ç?ç²apÕ¢?±""°ƒ>MIXED4FGL J1508.4-4817?ŸI÷cÜðÈ@!)éBNYÀ:·o¿«|À<°}á­/@ˆmm–±@!#=ò©Ö?ØU-XþŸ?î┵.J–@ÁÀÊ`@ùï‰:Pß?îïŠ1FÉé¿á{À nŸñ¿ç³"âz´¿í³Y(B¿Ð†0[<'¬¿ïÿæŸÜ©ºUNASNone?åF?	Þ®ª?Æl7\sÚ~?£à;lý?¤LØ›£?ÓÀï–GÍ?ÅI۞ÕKT?æ|ÊöTþ?ÆG[‹cmZ?¯n6§w?­uæôÝ?ÎF<>8Ž¬?ÃFÃܖÌé?ë&Š ØR<?¦¯yU"?¨)¸ªp?™ÜHx'Lž?º¶ã¦få?¡@›—â"?éP5âåèÓ?§'X´'a?±~!)V¢?žÁ¡–"â?Â0écÓ±e? ‹Ú¤…?Þi=ìI¿½?È#‹HP¯N?¯H©2±±?©où–¯Y?Ý­¬íD¢­?ÇÆùGÃÒÂ?Ù»‰\ÏR¨?Í;I'*L?ƯV±ßØæ?ĒÅõ˜?ÚìËI-à'?ÊqþñžN›?æ—*ç½Ç?¯îz:'s?¸4oSŒÿ^?¤jïú-Àô?ɉ¶f{W?©§@?ܳbsù³?¹AçÀ"åm?ÆÂۍÁ~?¹_Ñ¥‰R?×ë/Å%ʦ?¶&ó´ÃMIXED4FGL J1510.1-5750?ïÅvgO?É7ÑÌÀ8àpØ°/ÞÀ:DÄ)B@ $ÀS @ZQ	Þ?Â*2	h?Ѐ{zõ"—@	—ZYè©¢@0oz¿ïÁ­)«Ë?ï'ÄþÍ%¿ã ®@š¤Ü¿åxÜö¼6¿êk7@7¿å®7¶O²ÆUNASNone3FGL J1510.2-5754?½))'êñ?¹~u—Tò?Á>l額?¾Vf/\º?è?£¦Z??đv}"\F?°hqJ[s?±™òU®™l?¿6ÀpóÞ	?·}Lf\—?êÈlڎ?»iQä_vÄ?¾‡óÑ?¥Ñ ›5bÿ?Ç¥>ëoœ'?­}Ü´'b»?æE±ÇQ§?±>ZM#Ub?µ5Ävðf?' Ô<²Ø?½$}½ù=?œ-0#÷?é´·ÆðÌ? €©›ŠÙ?­êëº6Ø?¤ 4zqeg?Ğ].Ì¿?Â}‹ K~G?èùº	aä³?ÃýA¸öÅÞ? ¢Äwª
Ê?¡ÁÆOÙQØ?È«N!öö?ÄJÅZ+‰_?èñhå
 ?Ä2LRï2?µ²×ˆ['s?òjMù"?É"µä J…?±¶»ejŒ?ç÷•çø?²é¨+>€?™=gTýý)?váÄç·E?Ä)oîƒ	?©oìÞ mo?ê0Ji@òu?ªµu¥ñOTHER4FGL J1510.9+0551?î3é%ìâ@IM½ƒƒ­ŸÀ;IÝcpÀ<©7Ó«ä@ ¢§>H?þ7?öå?ÑWó;Ì^é?Ï
ŸÎ@ҘÀ¤ @¶ÙTD¥Ì¿ïùçýÕ®H?ïþY6Òúä¿Ø^m^'Rª¿âQ"ŒÂ¿×ÅÀÔqý¿ïüe"´UNASNone?ïض½
^…?bÉgÖë—
?Rt"pн?EœÀH²Õ?nù3²Zî?_
Åt˜ !?ï·C•£b=?}E
x&÷?X+8(Ö?bëÚú¥?~Sq
S»—?wbfQ@­ü?ï@à,G~?""ƒ'â"?r}´$ü		?s0Qk×cZ?"DnU,´?•IX¬z?îéþCg]Ý?yx
/Kó£?€R¯dYk?f,1ÇXZ¾?š–ßÜÈ8+?vr¨mä¶V?拓³#-'?wKŒé‹?gG*¬<±?_A+"éf¢?€
ˆ'M¦?rû•°Çë?ïÞ¯Aw?–Ÿ
ӵ͖?qzDI?z‹æc-ð&?™ ¸)¤*?"W&Ñ|¿+?d¼˜!?"'궔<"?€ím䄃n?~4¸Ìî8`?£+ž?JâŠ?ì¯(<®3?íP"µ0ùÈ?•»˜@)ñ?ñ÷¾7êš?ÀÁû/Z9?±½›_'ì?"H™'[äbAGN4FGL J1511.2-5803?ï¼B‹Zy¿¯ù ?{À8u–†¿¢BÀ9Ó²ÊÃQ@ ´<[Ðá/@C{~% ?Ö_þ"/T×?ÃWÿJ?þm…É=?ÿÂ+[xv´?éu^C,P¿é‹^e¿äˆHn-Û¿êÒåëÃº¿åm$€½ÕŽ¿ê¬ÄÉ$¢UNASNone2FGL J1510.9-5808c?ÁÎOôxÒ?À"k5"G±?'=ÞÑ¿ÍK?œÁ¨ž¨?êúŽõYf?ÁLÚ:ëÛ¨?ª¥VSXH•?²@§GԖJ?§qoS$3?¨qpNª?ìޙBó?¶ž"ù­?·¡fŔœ?¤RFPž?ºk×î"!?¦Íb2Ÿñj?é¾d0E?®zÓ}7… ?›Þ2°å?~†w÷7û?ö™yä ?‡"s2×·š?î1Z[sÌ´?ïÖƒX/?©>HêCo?²7¬þ€m?†Í;ZêŸU?"F^áã?îæƒÆãC?´+2• Ýþ?Ÿc;Ê—¦?¤S<.'¿û?°Ly'ÁwÕ?´lOâÕós?ìûVï6?h?¶¸Ü"x?³Ô£˜N? Š´®°Èƒ?ºˆƒ>/Ýá?§•¶ªp¹?ê4[%Yo¢?­hÃX¢?z¼Ü	ðµ…?fp$~-88?œ‡ñyË
9?"&h'Gù?îæF¼/¤;?"_Ç¥kjúOTHER4FGL J1513.0-3118¿åæÊ<
@6ƒõ@‰]À:Lm)ÏÀ<	Ä|œ2Ñ@ĐlIT]@Ý{~%ŸÍ?Ë®ýmS•?ÐÇ`&[^@Š#ÚМ@z6‡¦}?ë«6D_«a¿Ø	Žôúé@¿ä4߅·¿á'¼<[Ðá¿ïÿþ½à ¿?ï.°'kUNASNone?퀄!Ó?¥ŽO›k"Z?"ÿ\^S1%?òž'§½?­x¾áh?¢fŒsbÆ?íßZÀµ+?²üG
m—V?ž+ß#]õ?§]¦e8Þ?£HtbþR?§‰á ~?ìJƒtM:?£LZ—=XW?¥tÄ£¬r?–â7D+Ð?²ñ'—å{?›"kJ€ö˜?ì{,ˆ8%?"ìIÇ=?šÙa€"'ù?zð‹¤Ö'?µpC[ø¸ß?ÝykœsM?èì£b"èk?º€ïºÉ¦?°|¹q_Ō?¥IÊF²,h?ľûuN?¶Ú‡V%D–?ê‹QQù"?À¨
€?³­¤À¤Ç?µ\'¥('?·ù˜´´?±ºéƒ¦c
?æË$M‰˜?±Š"«Zh*?º"ÌœÀ€?£Ý3H#ª?Ǒ{yü?«ÛµMM?æQgñMW?«$§Ë­?°@ïÀÌ÷0?•i¯íß]?ΙèZ-.H?¨¨½j¤èAGN4FGL J1513.7-1519?æÀè¾x~Ê@A¢´A»Œ3À:õª®d,À<§)¥÷ß@_JÄIpŒ?ÿ×E|Y?Évz° F\?ÙÞš@
•ZÀ?ö@›R}PbÄ¿ïþÃT~–?ïÿþªJl¿ÖÔ]Ofo¡¿Þ´Þ. |¿êÂf͓œ¿ïñ.á"ÚîUNASNone?êü>‡z2K?µT…ŒáE?¹‡by5»?­YŠ¨—Ø?®1ŽˆÙ?ªì4Çâ÷?ì÷ˆ™­C?²ðGÃ!¥?«n¶jUvd?­Õ$}@{#?¥Èǃe?˜îed8Ý?êJ+ܖˆ1?­"Iy¥ñ?µ´ÂÁîé?£ÒÓÈ¥±ç?·ú›Ye¶Ž?¤-îm	?ꎳ	[u?—oÐâ?»õâ óQ?""«ng?¯)m­?Œ'-]´¥´?ç~Þ7-hÄ?½÷)ø?ÇÕöÙ³Ÿ?¹Èë.™4?´] –žH?®ÔU_áp?çåÒÆr%ó?Ä°ÔúÿÌ:?ÃAúÔЄñ?Á'"Œ
·E?ºMt"Íƃ?­Ñþ~­'?濘TRÆ)?µ9´±Só¾?Ãhn|=ñ?±"Æ!K¤û?Á™02wÌj?ªrV¶OoÅ?äeK3Z†?ª¥K2ì,?̶*žå?¨'ç'Yå?Á´¨•Ø;b?¡HžTicÇAGN4FGL J1514.0-6240¿×©æѬ
ÀÂ6ŸÏ=ÀÀ9Š»¬éØvÀ;6Û¿®×@S«šMÀ@WGC¸?Çê›ê¬²?ÉpNœ›+À?úzÞÞGH"@w9ÝÇEú¿ÓwÕd ¿ÖåoÛÛ£¿çUyC¸¼u¿ì"RÈú°¿Ôåî|b¿è©xŸNUNASNone3FGL J1513.8-6250c?ëÀўî˜$?Å­!œ¢?mû«¦F?uT™Qê ?À"ÊÕ{Ç÷?Å"QÕpñk?è€ï›ax?¾¼Ô¶iø±?wLFêʦ?AÆýµŒç?ÍEz	ÓµÂ?½³×Ž>È?ë/U0Wi?§Ÿ@M}*[?Ž.O	,Ãe?…Ëó·[ò?Á_Æχ½#?¦cyÅ:r?ì/¹¾Iž§?•ËÑ»y1R?qw¿íÐ?W
ü>q®-?½j¶XJ?•Pǖ²(?ä]=üËÿ.?ÆWteØvú?}Dch:Ö?t߶T?ÖÐrxeº?Æ؅Mî\?àˁ4ë;š?Çò1¾Ç"?''IGv?¹Wž#Kr?Ý×ÅÜ0?Çz€pí?åF‰º‡œ?´Ü"žþ i? ¸zJÿ®?'óp)Қ?Ó[ÝAË7³?³æõcú
h?åêN®ò?¬H ‰†N?‡<hcþ?vJøUŠ?ÓqúãO^ý?«Ûçۑ£»AGN4FGL J1514.1-5805c?ìÑ6'6ž£¿Ò"á#
À8ìÆ)wÀ:I¶>ëÎ@ É•½@Ï8ÅCk?ÄWŠ@
\$?(žÒ
?Ñ(@;Œ'?째Ex§¿ï¬^BUÿ?ïIë`á—4¿áu¿¿èŒ'Jÿ†¿àé¦A¯(¿æ֒³ÌJÇUNASNone>?ÀPøëä•?Á‹˜Ljô?š}¤aòë?¡âaü¢¼ÿ?ë$~ž…U"?ÂYwCó
Ã?­|Uøa?–æceš?£ýÓ\?£]+ºz&?ê#ÑÒRâ?Âhvˆÿ?ÀjI³/öE?¨Ž3=¤?ÃêÞðw?°vÑ;É9?æêíüFQ?³<D/Ù?»íɇ:? Æq{ÞÁÄ?£eÝë³5Û?‰¯Ãó!"¼?ëKèð*0;?£'|¬³X±?´ïEû¨P˜?¹S'y'?'6µÌ@â?•uCöeQ²?ìØa˜¡L?º:U7%Ai?²ö€W™¾?µBEÌrFà?¨Kòpñê?²ÂÌcˆu?ìpÍâ:a?»©Û¬Êµ?¸Ð+Ù8B?¢¼jp?ħ#×ò?²zÊßRY–?ç㻹ÿì?³¢AºàÈ?§‡*ágÿè?"S`[Q¸Ä?¥ê»z]÷Ô?•‹Yé?'?í(áš(#¤? î±¶âMêOTHER4FGL J1514.8+4448?Øòù}@L5BÙÏÀ9¾E	Œ³À<1¹[ÖÀl@
61u@­Ò^Ý?µ•¬O(Ý?ÅQî׶@Pó_ތé@ó̕ðB?ê_'Bd(Ÿ¿à¥è'
è¿âý ҈y¿æŽzí(8¿í-½R†`¿ÖNï|O0ëUNASNone3FGL J1514.8+4446?ï_œ_`}?‹Sê·ý?†á"N_²¹?ƒ¤4¨€H¯?[T‰J=?weË9(?ï·+Is«7?{®ÆðF{ô?^sQØÑ(?e³ò Bîy?|͆ݴŽƒ?t5^;^¢»?îÝ˒?••Pä?–TŠIY52?'^°ç›*?‹ä»‹$ï?'îI[(È?ïŽå‰î<?dÁM'$+?w›'6å'?Xý-Ù%Lu?€xÔçö6d?[‡Á}×ÒÕ?îX$ø:—^?©xèU0·? Ø«ú°ô?¢T-4Ëh?"J	
+,H?'I>ý¼Â?ï+&­Ïí¥?•| ²´?s'/b¿?€ÑÂØê«È?•¶©ü'4?'LBù¤Ç?í¬Ã¯´?¡uÛk¤}s?¨;'t=]'?žp<ÙBi?™ñ;"22l?ú€ƒ*éÏ?î½ø
é(?ƒ·~¶±-è?XBS	ž?uóÓÓ¥yº?—è¼KÞn?{Ɵ²AGN4FGL J1515.5-4242¿é¹''Z@)Zb˧2ßÀ:F;ÉÚªÀ;óò#žjº@€àîË¥@lè–Vîú?ĉûVxÍ?±Â2"ý¨?êVjÀh:|@üžîJI?Ҍùx&'K¿ål….¨‰÷¿ê@ý‹±yŠ¿âàÓ«¿è|ûhÁŠy¿Ö²#~4c_UNASNone?îšüÀ°^Ø?™è–ï՗J?zX÷š×ö?xl¾÷$†?£dþ?—:Ñz@ë?îZ~,<N?ªŽüåFÕÍ?'=H«Ú¹?ƒ¿:@ÚB?¥ÈËæª?¨lãMD?í>\`îû? )Üvf?"azÀþ?Œ¢þ[àÝ?±4¼^æKk?š{$¶6à?î÷Öã?ìá¾l#ú?'êë}ˆ].?_±—ÈGP?©…ÌÇõä?€6¸Êž‹§?ìÝƖk«Ž?«Ëò²9£?'@tÚàpJ?Ž'8"ßUï?´®Xzù?¨§Ç 8ÐC?ë­Pó/›?À^ÿX©ÿ?"†]4‹
j?œœÌxîâ?½sá®úK?¾ò¼âZ9?é€sG9>?°
9õ:?¦‹•°7,?˜GªyëÈH?Ä\¤Æž_|?«°i´Œ¤?êOÔõÌ[Ÿ?spé`Ò	?ŸçÛSÊÄ?€N΢kv…?Ã¯.	k?›‡y5 AGN4FGL J1515.6-5817c?ëôQR5µ¿á̓ ٔ[À8éŠÆ—ÿfÀ:'Œri©è@àØÏ›y?ÿ›¨g'¶?ÎçŽD%ô±?ßϏ_Yø?õ,+l•T?ÿ –H+gã?íu'}ô!¥¿äXYÐUî¿ç›Wã¿ãâæIu"Ø¿î]%uŽÛ¿ïîÞoŒÖUNASNone ?ŒÞ	52è?‡'dž¯?i£I*GO–?q}4Rmb?ït>·Ã?ŠE˜±)g´?Ð g>'®?Æëf©4õ´?£©þ¬óÝk?¢rA
ìÖ?æ¿áä$ò?Æ8eScL?ƁЇ
ó*?ª"â^'ªH?¿ÅQÌY?§™îƒIÚ?æfᤱ`ò?¯iÏÕÕYð?³¬"£½?§2'ïˆ?–ÀÓ>?§?‹ÇA•@?ìè	¬Úœ¢?¬À"åg¾Ï?‰ã(úb@Ä?'Ú¸"?lû³yÝ?l~(ý2ÆÖ?ï{x[RÙc?†¶½®Ü'Ý?ºÐà$9è{?¸hM7QŒ ?£¹^,œpX?¬SÞÏXÃ?ëjNx+?ºÒ¢hŽùq?ÃÀ ªÁ?¦$Þu…ù?»n/ˆƒÇ ?¤ ¯í«Û	?çÒ	æÄÖÅ?¬ãGêM±Ò?£	t¤Àà?œÔU©Á	>?˜E¸˜¼.?•…œ@û¹C?î
ѨçÐ?§o£(ž
ÁOTHER4FGL J1516.1-6429¿íYoÕGgÀyԀö4¥À:Asqç£éÀ;¹ë\ÚÌj@c¢fǵ@ë'Ü5ö\?Ôvóý=Wú?Ù%ñaËØ@R$ZR[í@…ÉêoJ?ï×"ÆÔeH¿àÛ
bY'l¿è÷ïÅöö¿æû	 :2+¿ïþ,@OÑO¿îôÔ#&vUNASNone?ã®f©Æý?Ä[?$€ñ?ˆÎ•Ö"Â\?~¬#Åd0?×ܽýôY{?ÄSü\'?ãüß³žp?ÁµK4öp¤?"2êl²À?'<­pÁ'5?ÖÓ÷ñ‹?ÁÀ«èaå?ê£ñ±c1?¨œJþõÍ? ÊÌD GG?'ÛՑ2?Á=ˆx×N¨?¥²2;ÃMé?é6óÿì‰×?šÁÆyðˆž?Ÿý AÓø?|]-Wþûè?Ç$|…&?™·¿¡‡Ë?ÞF©NºÅ†?Å	ÒÙl?"†ÇÉlu?‰#ßµ%œ?à@u =)?Äù×òůÍ?ՎʒN»i?Äq²0$œ(?¡©;`ôυ?§º/‡é`?äi D?Ĕt&ÿ"k?år‡Ú²ò?²¬æ†|ôW?­Øóüš?˜d¦%vº¥?Ñ_í8ۜQ?±5qY' 1?áhÃÜ@æ®?ªþzòtG?«3]"(f?"o¹=§??ÙÈ–á?ªøRt‡ŠzMIXED4FGL J1516.4-2640?퀠ÈѯN@9âÀÆ.MÀ;':ûÀ='ÛSxM@¦¢Ç•«M?ÿŽêéîEÃ?Ù¦û¢"T>?ïx?ânÂ@
UûÐÆW@4:¤ì‰¿íŸXàÁÌ>¿ë5ݜþ¨è?ÖȾË,d¿×wß4®]v¿ïÿëþ@bF?Ú>‰¨ŠÎ%UNASNone?ë|_ɶ@?¹TcàM?·IZ¡h?µ€åC*?ª
p¬À†Ñ?¤E''	kJ?ëŒÂ²±\s?¿\gR?¶s<@U¹?¹O¸sð?«îXùñg?£o³¢,?éS6L(ˆÆ?±mø—É
d?¶ÅJ­V?¦çáÉ?¾¡ïs•Ï?©ANNE?ílKW—?™§#ߜ÷â?ªIëœËÇ?"¬Ï‹«à½?žY{ëَ?‰C(ý,ï€?ç(°,¥qá?ÃÐÂE	ts?ÅKHŠªµÃ?À"ƒ=jLX?¼#í…o?µ¼Jވ|Š?åFKGD?ËðÎ^È7g?ːù¢mӘ?Éq§ü͊Q?¾­r`çî´?µ»‰«hb»?åE¶'©º?¹
ýf(x?ÁÌoãEgÇ?°°c/)T?ɵÒN/Ó?´	Äù|Ä?è»DՔ?µÀ,'&°"?ÂA™êï™ù?±lÌÊÞ?»6ôúk?©?x6®£þAGN4FGL J1517.7-4446¿ÀϘ¹þG@%w+#š8üÀ9Œ)s–БÀ;ÔÞ]	@³6	Qbs@ ò{²þÅ?»õÔ­ì·Ï?Á$HIDíp@hÚdeg@uó>#§¿Îú1^ò©«¿æp>Œ,ɍ¿ãï
¿[J)¿äÍLN+Í¿îM"¸aþ¿ï÷#M"MUNASNone3FGL J1517.6-4442?ìP»ˆí?¹tэI—?'6ñ	Á?"?Šjk¾&n?¸ìg{G²?¹ùÞÌÖ<?êµòþdÊZ?ÁéÜ‹/?°ø²KÃp?²OˆÿB–?¹WµÂ›Ð¾?¸º	iŸÑ£?ëÞ©RÁP?¥ß¿¹Vú?«€ŽNŇ?-#¿áÃ?³{u$ƒè¹?›B‹äÑے?ëZqáÕs?'N°ÚVaÜ?ªI"$ߪÂ?"} g(®?¸±|ɱ
?Š"SÎí?çwy^:É?¾(<xðñ^?´pՇßÇv?¬ÚÈÛH"?ÉÁ·V)=¢?º¸µS3ƒ»?åfcf#Añ?ËGxúè"þ?Â:VŠr­?ÂÌÖ+ŠK?ÈR8腐?Âá`kr?續Ž¡Ìw?°Ù8ð"O?¼æº½3ZS?¨?ƒÈ}Ûï?¢pfß ü?¥®¡"ðz?åw…6yþc?§œ¬X?¿7K"Ì? 	ÏÝY&?ʖO't9
? ÓòÈïN€AGN4FGL J1517.9-5233¿è÷ÔeX@'Š^"3NÀ9….mє³À<
ÇÚÅ@…BüÔÒU?þpCÊZ+Æ?¾q)¸á—?ãssÊÒ÷‰@ —¨mqó@‡B¨œö?ïü'-ks?î"=ßßy"¿ÊͲûÀUE¿ãg¡yâÅ¿î—;»—ñ#¿íÇîÁ"4€UNASNone3FGL J1518.2-5232?ƒBL¯ÙQ?ˆÂM1r?ïX ‹â]?•§ˆj~@P?†•[¾}æ?‰pGþ«Èï?¡k&!yc?µaÎy"ÀD?èđ"LÓ?ÄøÄ'óË%?È©žèk—[?Âzòh×s´?¡®
èSš?•Aǃ^Z.?ë¬
Ë"[R?¨Ë\'#Ê?¹ÈŠÓ:$?¥ .y´#?°*Ó×̓?¶¢'­z?êR¦?B^?¤Å=‡+?½?ú/Ë8'?ÐXD%#?tµÑ@Ît?{ž"+'F?ïp-‰o‰?'Ú[øñ?‰™´ð­¿¦?ˆTåñ!ö?Œ³%B
?¢k*è®L?èÆ<HõV?ȯáqAK?Ë%C¨Ã¥~?ǵExv›?ÿ¶Ð#Þ?‡
ÊõŒR—?ìÄ0à·T.?¤ŠD±Èªø?µž‹Q‡—?¢úûÜý?•€;ÕvÈ?€ ðú?ëqB ±?©Äcœ²}Á?¿c–õœÇ?§cpwPSR4FGL J1519.7+6727¿ëISno§á@EòxžwNìÀ;5Ñü·v#À<ùm"X9@ $©iuÍ?üGÐ^QÄï?ÌJ?(ßÈ'?ϵшžI­@l6|"ÏU@t§^ÿò?ï˱^²<ÿ¿îz´0ô"'?ÁXée´º²¿×¾Nî÷ð¿éJO^âäf¿ãׅøÒåUNASNone?ïrCOúa?©s®gJÖ­?pÛ	 S?ˆÊ•B¥t¢?‹±Ú"ã¿?£È)ŒÙä?ïa")p?¶ƒgÝ?|e*ÿ?xÊMd£?•š‰Š?‰|À‰·=2?îùHE5‹Ÿ?@¯Ê<âz?yÍnBO?{êFsĀH?šc³{‹€?Šê(€ë?îF›¨ñ?'厽&Å?'WÄÇvŸå?rz^›¹Õß?¢óÃß!êà?&Ðe÷?î´Ò-šÿ?š¢üªòÆ?ƒ¸'6Ç?xüªç?Ÿ‰¬pÁæ?—T™(hP?íÏþ"/T×?¥SQxÓn?‹r$9åÚ?6ÅڂQ…?¬#"ÒÜò?¡ð$°Wƒò?îw2oŸ?—ÀŒ¯´?†ÀÓÁ·Š?"ƝSzŠç?©˜Wåš#,?"ÐÉYñP?ëkø2ùsì?Ÿ듓CŠ?¡ô}‹§Ó?Œ_"÷.±U?»¥ÿâ™6?›£aÆ"÷lAGN4FGL J1520.9-3805?²xn@/÷ûH
ZÍÀ:}ke©¨À<#d"@‹ãJ<º@݊ú`"?¼+ö}ö%?°³'i#°?ñùYˆ1'I@¬ø¢¾†c?ïÿ™¾, ó¿à]d"Õ»¿é¿VŒÔ9¿âðP•CɃ¿à^Æz£4¿é9†3‹GÇUNASNone?ïz˜2CýŽ?"&ì	^e?VÙ9%;Qþ?L½­Zê\?Ž~Ì[/H?ƒrEš!†?ï±u#K<G?€Œî	"i?TÅFêIÞ9?ZUÏaqõê?
Oç²v?}Ù@LC?ﶯ7?¥G›Ì¯?v}ÈIÁ?x"e37?š(7ö2Þ?‰ºg,z€{?ï]ÏÔò"¹?h91ˆcëP?ræ¥(ׄH?QÕG¸Úá:?¸!ˆÕ–?dû§ö:™®?îîÅ¡ËË?–'‰ÀZ9?jH¤,Ç=ª?bÆC5©Ä?žÞI&-žñ?•'¢hüìñ?ï'Áñ?˜Bÿ©ÏäÞ?kö ðãó?i-L0³'?—‰_JÒÝ?•;ç݀ky?íÎê|h¹Û?›è:/‰'?‰b{ˆ'$‰?"0WØüRn?¬¸¹TÖä+?˜±·Òґ?î#CGÉ~?…ÉÇÖë?m)ŒN?s
 ã¡
ã?¦p…Y]ÎÄ?ê×È&ŠAGN4FGL J1521.5-8057c?ãåƒ2á
À3Ö/'4ø/À: ÃÄæNÀ<€ãÀ.@ÜaHÅ@¼@cÃb(?μz-È?ÃÏeÙM¹œ?öɊ=D
@™ÎwFÞ?ïó¤r:¯ÿ¿è</áoA¿èm`áAMþ¿ÖV¨ƒAh€¿ð?ï÷vG…UNASNone ?ïiZ^¸ü?'¯:3»?u$,Ÿæ#?q¦šR¸ôÓ?‹æÅ£6?Ñ"0ä?ïql'à2Ÿ?Žïoڛ{ù?r"eÂáîE?{¤N´qv?ŠbÃ2‰
?†ôѕâ¿x?î¡ñ<ìg?"æ}·‹©?ŠØÖ ä?ˆ6Ôì±?žºrŠ¿"´?xûÒ9l_?î£Ö	3?…ƒSU>U8?zB.gã9Y?a…‰qS`?¢zZù{&?ƒfé´à* ?ï¶P«ö?™Âáïý1?"Drœ'Ýï?'@«¬Ä¬0?•&ü¨Ž}Q?•Ü0!mÔh?îo;o T|?©hím?ï:?†Þõ""S•?•] _ªŒ:?£T‹¤a¿P?£® ×Jù?íF:†AV?¡yÛ³üc—?"âÌFÍ?
ՎcñÇ?°®•y˜U?¶Õ]?몸º¾yÅ?£"Õ7®?"UÍðkëê?õ½jŒƒ?½ÔÆ«Ëu_?¢zvH¹AGN4FGL J1525.7+1503¿îI঍@JOKD¢À:€øõJÀ<NúìšÈn@$¿÷t@öڜ™(?ʀµ^å?´C_Bå?çváfÃ.@V'Ìx"¿à'âLÒ¿êp'_ÀYø¿æ܀w¿ïÿ»6¢S|¿çlÊcfæ?ì A¾ç0üUNASNone?ïùWN'×€?HÌÛþ)P?!ût•@™g?%gáýNo?F#è‡ÉÄ?F"PY?ïŠê—cŽ?™ä€Œq+Ö?e–çýC¦ã?s¤M¼ö9Þ?‡ß æPÝ?—ðêR2–š?ï$T#©ä|?Ž1˜b´?mà^ý"?x[°C?—¹oÅ,;ë?‹Ãñ¤ ÷?ïÝVRœ?V½%﹚ñ?GÃ^«Ì°a?6`­7ØM?lùÒ7DÂ?T­¢­ñî?ïó]¼
è?Wl2ú?6àcùŒ+?={/4™ºO?SŒo^ÃÑ?SÝ²?î©z"¢Þß?²¶Ø¹êòÓ?um®SÄß?‹–ã<íõ{?¢¶IüÃøw?±³1¹>-@?îA?ýéFÍ?—s¢FãÖ?yiNÝ@?}©8%Î?¨¾Öamz¤?•d
]Õ\ä?ï}'sEÙ?}ñæq?†ž?c¬¹ûLj¬?Z"2.ëÄ?‹°4 !œS?zÉxY+"AGN4FGL J1526.3-4501¿îÁZ +üU@#XO	RÀ9äù8¶À;óé Àiè@;öófêp@ƦºêL:?¶z;°ZPY¿Œ•¢­Ù0w?ÕÁÔKFOp@'XŽó£?瘝N(ÿ¿åÁéå‡ó¿äâm©PÇ¿âø£JƒÄ¿â":‡»JÄ¿Îi{CÃ#VUNASNone3FGL J1526.3-4505?ìªúç|ž?°…ÔNxs?v¶¾
s?d«É608æ?¹?$LùHz?°nñ
+´?éÖLŒdk©?¿*<mô?…
Gà@&t?†²H²¹`?ÇUùQ<3?¾(êz?í8&ÃÊUà?›~.A!‡?‡/
>ý\?‡Â´t&?³Xè9|ÝÓ?™)ߤA?í|ç	—Œ?†yD$ø%ú?…0däÀR?b²ÓÒ§?±r»‡tî?…yƒŠí?èªÎÛÎP
?¸¬j?‹¬È[µ·?y"N‡?˙øNþ?·´Œš²½:?âŒOÇÇ?Ê?"[/ã?V£m?—‹ñP¿Ôú?Ùâ#¨§?Éë/×f·M?é\b…A"?«f¦ona'?—ƒ1}oz?†ÑSLḠ?Ǭ冂º?©ñEg"7*?èÄüÍn'?¡#â¸eom?Ÿ|£ÿÑ?'±ŸÚ"P?Èü{A–£? ï½ë›AGN4FGL J1526.6-3810?éÐԞ¨L:@.Ž­=%$À:ŝ%Ü3À<°ùïDÆÙ@ÊI±Nìø@l ºŠ«?Ê0pÍ¥»?å}¦‰l$ì@‰¡vݬï@-hŸ¦£î?ïÕ'^éšc¿â鏰â‹{?½Á]'çüS¿æ[Ûâ¿¿êíò·B!
¿ïæfÁ«¨UNASNone3FGL J1527.0-3804?ÕM^ÿ?Â8_½ò?㦠ӵZ?Ãû†Û?«1ê$IÖü? |k´ÅI?Ô¡ñ§w¨®?ÆûJª"^°?àG&Ðú.?Ç>µ…ø?Å §o?¼Ðg×eé?ÕòŠöWy}?²ÿÖtÍN«?á:°³í?´;óÇɓî?¾aƦdz ?£ëš°Twû?á¯xðp"¼?©›åãÄì÷?Ô̎ז!?©œån"U<?¿T"<Ñþ¡?šÁYက?ÌúxÓ6¯{?½ ™	ž1?åòÊY·?ÁØюŽ´Ê?¶z@
	­Ï?««wQ@•?Ämí2ì?Â
Yu<B?äùÚ毻´?É-w\'âÉ?Ǫ§Y±ÞE?Àª5út&?ËÉæ#Ǻ?±—¿{ŠÎ?åf¨E.?µVÎé"?½;îvHdP?¦$¤î"Õ?Ñ[Øp€£?®'8žY\?àng.ëÙ`?´Ãt
H@Q?ˎ²d/™:?ª±¾Ì«€&MIXED4FGL J1526.6-2743?ãH(zóf?@7®8ûÊZÀ:³*¸:n'À<¥Ãiv¼@Mâÿi,>@mæh3?̎BM'iÒ?ìq='‡­@ó'ªi@éR ‹Ñ/¿ß´[ÜõŽã¿Üυ
ñZ¿ÆGçà¤p¿äšyޓHÈ¿ïÿÞý¦ßR¿ç#î¢	ª¤UNASNone?Íüï
ƒ: ?½ú¬L,\?åsøwlë]?Á¤î23j!?¸f^*nÕ?«úbu)ȇ?¼]q +Y?¹.lüŒëÒ?ê-iîcÓî?½_Û6òÛ?²7>ê"Rx?¨‹&õnHá?ÍûÒ£ü/?°Oô5¬S?äW_äÛÑ?´Yj­Ýn?À¦®R쿏?¥œ?ôÖ*?љÛo
:6?ª4{¨Z?ãâ‹õÅ?®ãûX§?º":Si? wSiK­"?Ápò¾Elé?±Ú<g‰?çôù^¦(ž?½ÔÞ (¶Ð?½vOŽCá=?³R‰fèä¨?¨Uìü®?±76å#Ú?ìrAïl<?¹ØNhÌOØ?°C!ößjÀ?ªçuÄ£³?½®ˆK
ê?¨9¶õ"ù?èP@µ°Y,?´b	ù<½,?¿Ïr'§º?ªeܱ8 ?³œÿd* ?›>n©±Ÿ?é¿#'2°?­4€$Ót?¾þIÇtHQ?§}úD'˜PSR4FGL J1527.3-3103?Úü4É$;@4ñá~4¹EÀ:åJrÀ<%1ðÃ@ú"\ñrŸ@Õ7ªÉ?Á·]ú²
Y¿"ÝLÌ·S>?Ô »¡×+@t³Pw¿ãÓÇÝúœ"¿ÐùW¥ƒh¿ìUŒŸ
FÖ¿á­IÿþR¿×Ōf«/ĿٙޣcòÄUNASNone?ïë7ñß?"êL×¢}i?iä´ÙÇ=?b,¹B¦­?™O«þ×=?"©–}4¨?ïÄÆE6?tp1 f®?LhÇ pz?R^Áâðô?zöµ®ï?qóléù0–?îw‰¾Ÿ?™&ä‹Ôa?xןË?zPòuЪ?¥t+g`,(?—Êè"\?ïuK,_j°?išžR7®?R+CÛæ?9\[$ݽ²?3æ/¡½?h¶Ð½Aqi?í«½þL™?¬F'z_n?…–¸ò-0?j=w6Á?¯Þqà¤h?ªnU8º³?ïj!Þ`?®О¨?ZúåóL2?e×SæÀi–?'ðv¥B?Š²ú¶Œ?ì¿ãJ<º?§QnQý?‹gÍCµÏ?‡~WÒ:?¶š+)¼v?¥0MªÌª?î?ò> w?‰Ã¥†·¿Ÿ?n'=빎?_ û½™Ì?ª¸N3ÁX?ˆÕÅÐÌd1AGN4FGL J1527.8+1013¿ïdógÉÆf@HÁ´xB0ýÀ:께Çâ'À=ÏZ@Ѧ¦G}@dGšÉD'?ËãŸ6¼£?ïþå-7@''¡.¹Q@ÏUï˪c?ïöW	ÒÙ¿âô8ñ
¿¾Ôw»ù?ò¿êõ°»õ4¿ïþÈÈ[N¿íº(ðºßUNASNone?ÑçZà©×?È\Ñè¦Ö?åJ÷åKÁ?ËLGÝ jÕ?¬ª¥õ6g?¨P Ɍ?»éœÁ?¼i…ˆHA?êMÌFj©?Á°›Û?²r‹áÈø?ªû
«MñÜ?ÙaPDŽ6?´Å½e
#?ÞVå
l{º?µY£Düi?À•cì?¥›²
-åì?Íð•÷ ?®gL#w²?çps§[gô?°XËՋJ<?¤Å*±ùE?"×ä4UD?Ë·3vÑæ?ÁJT3?æR^^ÛÄ?Åm\~•?µþ¦ßÌZ–?¯ÄêJúÌ?®h©ÓÈ?µA«kà,?몝§½–?¿''ôoå&?³v½Ú=9!?°$‹ê¶@?ÏÐ~¬H?³ntˆÛ4?ãí)?®/˜?¶röpð?ÀzÜTª&Z?¦d8ñ?«QFD?œ¬Õi1%?ìÒÒætá?¦FG>ÜHf?§·€[ñGŸ?œÎÝæSTPSR4FGL J1527.9-4943?íAÿ©ÃÞ<@š¬"¢ºÀ:N õCÀ;‰Ö,Çß'@"zvž˜@öuÂú»ó?Ϝâ#v&Î?Õ§IEbø@†NÜ%´@£E9›N?ïÿèã«6¿ë3!à¥q¿¿ç·€4mÆ¿å9ÞHT¿ïý6âjBê?Õ
‹ÄCç6UNASNone?ÑHÿúe?Á¼>¬…{ø?'ªÙ@Ñ;ÿ?yŸŒ¡[Sg?çO
·×%?ÁæÆ	Üo$?å0ééþ?Âܽ•tF?¦¯nïîá?¡ô¸Qª<‹?ÒÈ>i‰-?Á
å†
º?âÇ®–ð‹³?²…þôF¡@?°[š×ów?›©bה½?Öl‹ì)UÜ?±€Æɪ8?ç»(EՈ?¦ Ê"¨	?¦Ã¯c"n?ƒTyRöø½?Î '}ÔÂ?¥ˆ÷Û¥Iÿ?¾çÍæõ[?¶W¨5"R?Šˆ¬«Qú_?†"óÃ|Y&?ë¸ãªÿë?·N7+^G?Ö¸!§ùx?ǎ%"p?·€±^ÒáH?¶€,1͇§?á³Ù6܋?Ç1Ï2$6ã?Ø­;ƒ?²<íKá?·ºkPu? È§‰ß—?áhõaìY?²ÑñdzŒ?ÛÅÕzxõ"?±Üàiê?´{fŠšð~?˜¢ð 3/?ßPâàNN?²°ªÈºMMIXED4FGL J1528.4+2004?áD¸/ ›Z@J¿
=p£×À;møDøÀ<"ìˆ3@@ $¼ev|^@¢€…Ì];?Å«®o´¿¯ûÄÃ$=³?çžQYŽç@#+¿÷Q[?í¨)µ/ë¿î±
õ´M?œÄ1%oƒÏ¿ß¸ªŠ¿ãbr†/YŠ¿Ø#lÁŸG.UNASNone?ï½Ëò 2>?s€Ådw?P'ìJíÂA?Oé
>K?|ùK÷ød?qkeÏs¸b?ï~À>ÁS>?Š{H>	?e½A!Z1?l–1	Âà?ŠàŸýÛ©?†&~iÉd'?ï/a(RÉ??‰çDŒÝ?hÃìé¡¿?q¼í,¥ç¼?—BrŠCã?ˆ€ïLÒ·?ï'w3ÿ?x/p¯5O?g«u:+»?S"¯jyæ?˜®š"N¶?wÕ¼òN'?ït9PŒ=?"b,¾¤"ç?`ËÏ'Í?SÝ|k!#?Ž¾¸'T™?ƒ{•Þµ=Ë?îÆÁº
ò ?¡Ú†'Oæ?qIeꢹ?v­ù"²?¡j·¦Aj%?Ÿ—æô½Âô?î"k8w±?"C'4"?jU
Ê–Ð?g] –Wž?¦ûÈSdƒ?'­mì)¤ã?튘Y*?™˜É
pC?¸-Ù¯Ê?vM.×ü¶?µ¥'ØxW?˜x"Ô°­AGN4FGL J1529.4-6027?æ>l'­õ¥À
ª'†VƶÀ:wP™u‡À;+;íìØ@cN€ÌC@yDàá6?Ì0_ïÉ|?â)ñk@«ýq°F"@ü¦
›I?ë–åõ'¾´?ä	Ñ¥y¡­¿åœ,ñВT¿éËÕ¡1¾i¿ëîjáö)½¿ï#ˆÕü÷UNASNone?¸Ž½F¾?ªïyÂ&?«FK©K¾D?£´Óž›&?ë9ܼ'¨?²qêÐH?Õzúâß³¯?Õ/€åÝY?¼~ƒœ4Ý
?²¶$—¶€à?á²²€(?ÂíÞü`?Ú©¥5.5?²Pužž®Z?À«/Ÿ'š?¦|5dùšY?ÝÂû	B–?²¹*j±?Þ¾šk6ì?¤LŽø
?Ê>n`ìæ?¡eö
úE?ÔÏ
5V?¤óù¡wE?£‹Í‹á
¢?—‰5ŽÑ@?¯óB
<?¦Ð‰[àR?ìÈiaÕ?¬'¬¼=æ?Á?þ:á…õ?¹–_~Dó]?Âò°
pÎA?½³°í¯V«?æóTmëjó?¬(¥Ä'ë?Éiðÿ±üg?¬†b¢¶?ÀëªÛ
}?ª"v;_kd?åj£Õ\¾G?³¤e(‰\?ÌöãÕ/¥h?¤mZžÍ"/?Òø¿) 4Ô?±]ÿþÙ?ދÎìGøx?²íïyx{MIXED4FGL J1530.0-1522¿Øù8ƒ="@@V¤"‰—ÄÀ:°úìšÈnÀ<Ò¦*¡"@ÎÝÉl@žnëp&?˳+;-C?ãõÄ<ÛS@¶'ö @0W`¹ÿ?ïžæu¿±'	/(·"¿Þò¢¿æX~FVüf¿ïÿÿ&¦³?ïYÌ?SŒUNASNone?ßRvÊ·ž½?Ål^,Ü?Ø¥€"ƒ?Ç|"Ë	ºO?Àa›€?¶uÑ­ #?âC†zá{8?Éa7Â'ñû?Õr7;8?È(•çC¬¹?¸LRa?©É_ìÀ+?×aC(–¨?³>ën$ß?ÜTUØ#Âþ?³Ü‡¼ã¥Ë?ȔÍüf‡7?­otw¹.'?äx ÿî§?©éªhžÏä?Î%Ñ;؄w?§TÙXóÍr?¿óUˆÙ¿
?™( §â©û?Ó µ_ÑTz?ÂÙÐ&¯¨`?à*A"Ój?Éx¦å‡ƒÂ?È\7äGé?Àá<O½?Ñ'%×2´ç?È,vß
Õ?ãP,¤_¨?ÌÏï0?Àq½øÒ?µAÆíçY?Êϳ"	Ô?¯CV¤£ú?☬·a?·I*"º™¬?ÊÏÐq`Ú$?²v~"W+?Ô'‹h²?¯
kqèü?Û&nÊ<¶?´ìþ_È»¼?нycªZ˜?¬:鍇CMIXED4FGL J1530.5+5850?ànŸŠ±@H
r!…‹ÆÀ;0mWoÈÀ<­
‡¶B@´×xÍFD@b??°ï÷?ÄzIÚÕ¿¨ï¥È /?à>¥ÂœÈ"@çòiÇ¿â"±?¨Œ|¿çº=³¿µ¿ék¥^¿ÿ¿Û"à?¿ïüc]j	?ïŒËà"©UNASNone?ïå¸uÊ(û?cw¥}¦h?SƒsþW›â?Tê/K®'m?`…Ð[Æþî?ZO"EÒ\+?ï–#†©
;?ˆ«Œ…¥Ú?b[³ªpè/?l•FèŸÜ?…à1\/;?"xD	o?ïO|Qà‹?ACàÌÖ?q¸ŒV˜› ?k÷Lhë|<?'¢R®VG¾?~[M;¶a?ïÕkµcWF?YŸ³^C± ?Yhg®¡#ã?Fq"Ç	•¢?mà㔷ú?S#«Ñb­?ïÀڈ¢%"?ur<Ÿéý?k7÷¶+ñ?i†mbô?qö¿Ìøƒl?lÊf"†…?îÅxŽÆà?«¼­ÔI½?q"Ε+ A?W}°$•?¡v6gôp?ªU>,ØÈ{?îª`r JR?i©R?{r­ÈEÄ?sH'»¦ö?¡ë¶ÿ¨c®?Dþú«ß?ïX.œ9uÜ?€'}gR(P?z8ðqú'ª?o•$ƒ?Œ×௶D(?xê¯R|AGN4FGL J1531.6+0406¿íËñ]OçI@F³åBåWÞÀ;VÔ"+¤À<‹Øž'&ß@
8=3<@Èáž)?ÎFacGM?ÃŒ¨šhw?öFl{S]u@W‡§£?ߪ_d"(?ïñgìxc¿¿çeà"œ¿ÜâÅB>ê¿ãžzߚ.ë¿ïÿÀ?ЀUNASNone?ï·Q‰ú.?p&XÝþT°?UôläÝÍ??H‹GÏ&G?~Ú´céñ?mX£†2®±?ïÉUB–lW?tڎþÌSt?Paï̵״?U@­ç#Ñ?w<âĐÕ.?q<M·í?ï…L³Àiñ?x2±ô4?_Kà£û9 ?Z–«9{?ŠÃW† ?vçÛ»Þ'?ï7Ü+J­?r'²‰O€Ž?{	á*Qã"?`iȉYÐ?'BR'‹?n×?ق:?ïQc~á†?""1"mÛS?i>y\•0Ä?_Ԝ°=Š¦?'«Á=?'ÃÏk¦­?ïNŒ‰ª}?˜Ÿé¾æ&?cLÁf̙Ÿ?lc¡ExšÇ?"ÄÖ¤¶?—xmù»j?ï¥1½?….³b;¶?iü5ÈŸ?`Â_''Ö/?™ËÓ`óg?ƒÓH–¹–Â?îÅY³G?a#JKÂe?w
éÒµþ?x´ÔÕÒ&u?¨•æézú¿?‰3¢7ADAGN4FGL J1532.3-3857?ÞÞ4dô@+ù"pŠ¬—À:Ò«>݋aÀ</"Bð?™@عó¬4§@Iß9¶Úó?ʽ	¶74?°"ŽJ[?çÉ[ÉTrH?üùä]K?ïø¯^|ã¿är5<!ï>¿æBµâz‰¿â^06ÿpŽ¿å'Ë9NÖ'¿ï×G²JkUNASNone?îƒ"ÐÅç?ž(†Œ®Š?`)̲'¾?V,ÿúåý?¦Í:ïŠÔê?«"y?í˜ÑfJÈâ?±—¬Yý±Î?…ä*¾Bç?…ý1b†Z?°‰8H¿ä?°Œƒ'œ?î‡òÀÚÙ³?"€9ºû'Ý?{2Ñý ò%?tøÒß=l7?¤yµÅì€?'0Î`?í%¾þ­ði?‡€,0¹©?‹kshñ'?gê¶îšL$?³d™ŸELˆ?…îö+²ý?ëËS7àl?²½1G	y²?t"%iƒ•¹?nî•çãʄ?À.ö¢‰,?²x—Z.?éÚ¯•õS?ě/ô¿|?˜`ɅÊ?¡%d?'n>`@?ü²kìÛ?ìV5'\^P?¨nE3äÿŒ?%èýG?†ŽÅî?¹DÙqŠ°?¦s5¦±ÙL?èmLÇf˜? kf6‡ÿÓ?ŸÿM ÆÔM?""<‹æ™x?ÊJæVe–?ŸC_ð
k9AGN4FGL J1532.9-0313?Çq¡|€È×@DR)AAé¯À;Z4ù»À<ʽé:ø@4ê˜d»@¢®Ñ9C?ÖTéf`‡)?ë6ˆ™"º@	 &5@H8}õÏ?ïå²af¢K¿å±ÏñD{Z?Ók—}µk¿ç¹¾!ä+c¿ïÿ¿h`;ª¿¸_ô‡PíUNASNone?êú‡çÚ3,?·8sªjÎà?±&¯²¯?¦Àñpqâ?·
¦™¢Ìö?²CØ'6	X?æóYxŽ©s?È^BøÅp"?Ɉ;3˜ïâ?Å©õ@x/?µT½Ó|í¦?¬
ĬËX6?éò›
À‡?«êÀ&4Œ?µ¿{2ÙÐ?£©~šãç?º¬&È¡ø?¢æ&ÊÏZ?ä'U~"à?®^:_+Çu?Ðl;—Û©_?¬Ê99ZŸ?½e¬pû…? EðŸñ¿¤?挋"XÖ?¿ƒ±GW¤Ï?Á™…™ÿ½\?´sD.þÒ ?Ä4LŠßJ?·ÀÎz—à?Ý<Jov?ÐP£_¢?ÙZ°%ÞG/?ÐÆÄ`¨Èr?ÃD'}®'¶?¸~°þa?æ"í¦È<€?³q˜ñv³?Àî-µh`?®Iÿ´rç=?ÄÂ×)¥ž?¨‹•€n?Ô"ø¦MÚ?³Ôû%®C?Üõ?î¾ ?¹Ø
}‹'?φ$3ˆe?³zZ.â¦MIXED4FGL J1533.0-6239?ïÈ­øeÑÀ†¯f•À:w
)´.pÀ;¬;Oag#@ȯ+|/¦@È˛te-?ÛÜ:¾lâ¬?í:û@
þ
A¢a¿?þì¸"ÁE?ïâ, GÑ¿Ód~d‰íT¿ì&½F¿êÍì‡}7c¿ïÿØ]#Dž?ëÛu<Z#UNASNone?ãÑÊ?Ê÷dHß?¥õr'L»"?£¥pçnš°?×®'ή­?Ê\áQò?ۈ·Sé·?ÊlEî–?»ÎfY?%I?»·=eÞx"?݃¯Æ›?ÆT÷͛B«?á7oGWúµ?²K°^îR"?½¹"OOq?¥´ò."ã¸?Ö"ØÝ|Gy?±äB³y±?Ô«
¤CF?°C{äS±k?Ùz4å\]?³L: èKç?ÑÚî(A?®"˜éE~d?Þ²DªmÁ?ÊQ¿i¦¦Œ?´$'K:ž´?°ýh®¼¬É?ÜD–Âú'?Êâ[¿ÄP§?Âò	èa'ã?œJµÁÿ?˳æö û?ȏo¶¾ë?äV"*-È?ÊÖN"DE?Ø)¹ä?²ÜåÅRkC?ŋ©Î½_>?¬'r&1CÏ?Ý"—"–}?³w¶¸ò?²»ôû¼Ã?ž¢Óý¡?ál#& ¨­?Á#µ`c[ß?Øx¼s}?¿§(߃nñMIXED4FGL J1534.0-5232?í"í•Å$@QÔ=ÚV"À9—$tSÀ;NѼÖ_@¨a3÷~Q@f":Ì?½-ݳÏи?͛ƅ
ƒ@P +"?ø±\"±*¿î	\Ý°Ë?ïûPÙ6g›¿âÛÏ3¯Yõ¿ãðV+Ü¿èÏ}¶åû¿ê'úhçJ'UNASNone3FGL J1533.8-5231?܇Ê0Ð?ÑÎO"ùÞ?»u'@ٍ?°¼ki{0Ý?ܛªe™·Í?ÂYÕ1Ræà?Ðkþèö›?ċ+fO7?Ìeüobõ?ÁƒLt¼"D?ఁo¬5S?Æ1äc?áîIŒeÿc?±ÎÚÛ7±Ž?¸
M˜Õƒ?¡×ëôœ?Ö lX?°èt`¡–Ã?ØL÷øY?¥€)í
?ÊJFö°?¡*˛~ñ?Ú°ÍåsO?§ÆÕƒ–?żÊÁYÒ?· J!‡X?Ñò"•ôs…? }n?΢?ᗃ"¯Q½?ÂÅ%:JÃ?¸'û¨~û
?¶ÛIZ¢C?ÔAuœ p_?É#*¯'?âÌå¼1ôð?Éʆr0°2?Õ||)ò?²Mñ="Ù?Ãûxözµ?©yäãèôÖ?à|9[LZ?²–"ò—ci?Çf*"Š?£!ðÜÉ?Ҙû<Tw¯?±"ɯ¸Ž?àïè×U£?³OW"%;mMIXED4FGL J1534.3-3312?Ó꜍â"Â@2WÙÛ©¢À:ßØy©9JÀ<~Ú©.b@‡‰6õàl?ýL¹ñ'ö?Ñ»è#'?Ýp¥°@
E^³¾@oµ9Þ,?í`L•ÚȿڅKCuJ°¿Ö…ÜãÆ8‰¿Ú'}keª¿í²Ûe¿ïñn7@UNASNone?ì:Z"KÒ?±^¡PÜ·?°@Ô µ‰?§B¾1êó?«Ø¯¬qÓ?¢4»ý'Ñ?íûU†oE]?£mziÄ
?™ìüÁQÜ{?"¡ðÈX¤?£T):‰í?™*'Á6€@?ì$¼Ì?¦MvÁ­~?°&ÖNBé?ž÷É—å??­f+5ß?˜­veúë?ìM¬jE‡ã?Œµ\1ö?£cò—¾"?€dŽ.Q°?³à£ +ú?†Y'â½¼ô?骣W2–Ö?·sÿ'áÚ?ºò¯cʬ?±e">bá?·¸5å¢Ù?©8EQÿã6?êíN@ą?¹@Ø7Ò
Û?±'ãéf9?±ºF²µØ?·ªQ…0?­Y¬6%x?çÏüª`a?µz@åð¬?ÁœÚðë©Ì?°²WÃ,ÝP?¾FdË()a?§RSՂ7"?ç"$yé?¢ËËÑíK‡?±Å»‰j?—è–ú$k<?È̒pÁšP? ‰"»SìAGN4FGL J1534.4-6719¿íeE«)ôÀ"ÞøH{šÀ:ª'ݽµÙÀ<9v+ÖG @zJ''?@(:6?ÎRçÃô*?ÒqÁä;~[@m^!ôFŽ?ù´à‡iÁ:?ïæ†è¼í?ëP›ÄDæ¿Ù?""Æ¿äHcUeb¿ïük 	ŠÃ¿ïÿÄ;-ÓxUNASNone?ã¼H'X:?ÂTCŠT"f?ª¦OÅÇO?£xQAÞi$?Õ2¤âð'?Á-8I"ë×?Ú( Þ¥oï?È9ƙƩâ?¼O"®Ñ˜?·Hd1}²?ÞļnÛ«?Ç wj€ã{?ê#ë¢Oö?§¥ ©q=?«3HGe›ð?˜'Q>?À£c.ðÑ?£Æ`Üjá?ã'çÊ¡pË?§õX.°»¡?ÊŸ@¼L'?¥W†e–?É^Á"½ðD? "~õ~L?Ö\·(m)?Àt†dSD?»sŸÛŽAÞ?±9¨Ò	3?ác¨ú0?ÁkL+tz?Î%/?ïÀS?Å¿ÿ»GÐ_?ÃÌõ˜R¬?Âh¾|ÊMc?ãƒvʌ« ?Ê\K¹5ý?ån'D‹å?°s+	‹?·uæQ9JÓ?¡ÝvÒÀè?ΊĴÐVÅ?¬l±ü^WF?Öå%¢ë–«?®¨|{õœ?Óˆ"4?´K±–O?ÕÿR9Íoú?°j¥JnòMIXED4FGL J1534.7-5842¿æ'ÚÏ*0fÀRzÊÒÀ:¡s¥ê	ôÀ<–:º1¦@ 9ʆÌbo?þð– ÀÕH?Ò)0æQÙ?ïþ©Þá!n@kpüÂ]Þ?úô?Z2üW?îôÁrüvß¿è
þraF¿Ôsíw¿Ð¹PC9e§¿í²UB&Á
¿Úk ÀÀUNASNone?Ò¦‡úÆìI?⯠t²¸?ÜÓÀ~W@P?ÆLÁ•á©?Ѕ·†áÓg?¿ª}Š¢äO?¸æ²±?»©%µ"—™?Óá3U[Àà?É%&Ka?㣲LBú?ƒ¢,mÏÅ?Û ë#
WX?³±bé"Q?Ö,$*šˆ?³ùwµ/?Ìeᙖ??«m)™Äq:?ćï\2Ÿ©?©¸@uQ?år?AÖ±t?¶t³•äÆ?ůœrš…?­éû?ÉG éL¾?¼Â
ë°,?Ú»|ÃJ?ÆnÃ}ÔÓ=?ÙTUô–W?ÄÛV6‡?i?™¯C	Ǭ?£ ‡ýy?ÔJ¦ÂÖÕ?̱ó5Iìf?å
2â¼ø?ËDž+3ƒ?Óý_t¸AX?³Óí`ªµ'?ÛGc{ûN?¸ó)i'X?л=Lp"?±kgýº+?¢›™Ôü™?•ª[¢ä`?èøóÕ¶f•?»Ô=ïϱ.?ÇuJd¨ E?¸ÅKFÿ¬MIXED4FGL J1535.9+3743¿ã\1÷tŽ@KNã'áïÀ9瑳ò
tÀ<"âɎSë@–íÐÓl¤@™Ãیƒ1?µ
A\Õ?ÉiÊßaÏÔ@Ï8ÅCk@ǯPY?ïjøœ^oø¿âûµþ!s¿âOX}o—h¿ê«³AáKà¿çv"|#g
¿äk_ý–™UNASNone?ïæ9½2re?^û@Hï?`£S[rq?XåšîêÂ?RFJ¤­`®?G©T¢ˆÜ?ïǧŠi{?v*Žp‡Ú?S)0˜Ö¨|?^¸M^k?wb3žäl\?pï'GҞ?îúÆ_J?"+"Í‹ŒÜ?]u§ûF?­ïaÙ+-?_Vö³…f?‡h¤ó_M?@ç.?l^»ºe?q‹C1"d°?V|
Hø|1?ƒŽUõ~=?jq]LK²?ïÐ
¥( ¹?pjÿ?;?pGç¶`?h˜¶¶Þ?^ËÛ®½ô?X†²Ûu?ïO›óØÂ?'·ËOú2?ggÙQ™<?qDÐbX7Ã?"*4'öë™?á8˲ø?íÛz	[sn?¡^ñaˆ"i?¢º»Çÿ¤	?›+.Nß1?ŸGA"®-?'ëbWíø?î2öžœ&«?'ú­õ`¹?"]™Œy7´?Ú^;Å%?£!ÉMmDr?ÔبÛÓfAGN4FGL J1536.0-2729¿îƉ"Xï@6"9:´0õÀ:×ÌQ|ÊVÀ<I"G!þ@dš½."@¿]þ¸Ø#?ȑ²ZÙ.?©󼥸6?âȕз=@rƒ.H<Û¿á#bp7 €?ëì²ÍOÔ¿éj¡3–Û¿Õ6—;~Ü¿ëé[x̚x?'E¿&ñÜQUNASNone?î¯%3/:?—o©œÝ?rûé²ñ
m?fΏ}'?¢®/"ø]?–&ÚLv­?ïȄW‡?uïBY #?P"úȐˆ?WgÔ¨Hëû?w˜y€kí†?ró0½Ñ?îù"Ï…?ŽmÇS(H?toþÆg("?q›¦ßß@p?›¿¦qäáÑ?ŒI_׎B?ïDQçåh5?qªÃWšÒ?p˜û̃§?R]nq×ñŠ?"O"Š*«?ožÒp'=Ý?í]æH&'ï?¨

þÍ?ƒCÂc›'Ž?yb—šÕõ'?²¨Ur4?¦ÉIn4ÆC?ï_0†8F?–Ī[· ?b	p…èÑ?l(J®Ô?'Û«Ûè(?"ò³zX?í¢ÃÕØ9?Ÿ"+ɾl»?3lT<?{Š®ë 'ƒ?°Ë;s»¼ï?JǦ‹?íøK5?Ž-<ªÿhC?…¸ÖE¹??pÀ§¥lª?«
H?Y¾?‹|¡ÍUïÝAGN4FGL J1536.8-4327?â¼#±#è¬@#·ÃøôõÀ9­‹0JJ§À;¨#ÃS§G@¬º†¤ƒ@™åóí?ǵrþzCé?Ó4# Ál@€IÄo0:@/¡¨Ü­•?ï¸\Ó?­•¿ãšµùK°Ø¿ìpgÁ°9¿à™¬cû¿ïÿ݀y7$?ê|'œýÒ(UNASNone?ë¿5w—?Ãg[T §f?÷wg·ì?›ˆ§­c?¾GhŸP½³?è©éJ?ë|!åÃ?ÁÑð—q?«è•®ÒÔ?³x©œâr}?¶+¤hgý?·K#.0Õ?êÔ!J'–?§îG߈S?¦'þÁ"õ?™¡ɓtv?¾RøÆÐ?£nB÷7?íy-ØK?"zä(²F|?¢JÇ1SöQ?"á¯ð¹Š'?­¥òâBý?‹Lvms	³?ênW‡·€?À—Ø[B¾8?¦yfþ?§´ZÇïã?ÂB½aA?¾-ÕÕxܤ?å¨æ­ëØx?γÕ;þ€F?ÁªôÓڐ¸?Ônϖ?DZptv
g?ÄÛ÷±–ª@?æø@'ô^?°}ìšì¨?´'ê8N˜B?¡†5XS¿?ÉՈٿ	Ò?¬'h¡?…p?åʲĆ?°,Oê#?Á©´±opž?¨@W좖s?Ç."'}I?§J¿×E÷†AGN4FGL J1537.3-6110?Ù
^g¿VíÀåë`5ʽÀ:¼înÞ-À<5ÈÝT@9ג"­@N:Wê£?Ô#";9?æþ
·x§²@)@þÍÐÙ?ú¸6OL,?ïýi¸*~Y¿æ>
ÝS­§¿Øðh]a…¿èWJ*,¤¿îÓ6=ª¿ïȀâ¾|UNASNone?Ѥ¥Öí? ;«?ÁmÊD?µÌœá¼Ò?âç­^{$?đwG¤?Ñ-Úüî~?Åkén$?¿ýÌðšB?¸×Å©/?ãiXãé@m?Âd~§5?ßLðŠ'qð?³o¤î*xK?È÷v'?ªî½´í7D?Ô;K®\ÒÇ?±a¡‰¦Â?Õ×Lrÿý?£yj®'[{?ÕG²~p(?¦Ù	#Ⱥ¢?Ôáu~Ü?¤^N†I%{?ÁQ¸ V2x?¶:MÃR?Àç
Žì?¹~—D0¯Á?çqÏ4ÓhÀ?Áé¿éíø?¸ª*RO]T?¹ä)W3ºå?ÄqåÝó?Â,d.u*Ç?çÎt|K!‰?Ã1׏.ÂÇ?Ô·Ä+W`~?²xõ¿r7?Ðú
^þ"?´]Ôm•?ÚN,É6À1?µÊ …?À'ßz=L«?›øub¦¿ý?Ù3º0èÖ?´#Zܜ-?ރx‰ÃQ"?²ú"€¿uOMIXED4FGL J1538.0-4638¿ìÉGß4$í@´À>IëÀ9¥£×àýÀ;V$fÖ@Mj¾È5@k#Â|ç²?ÄK9?ØÆÝ"/€@͌ƒ"_?÷΅Sç]È?ï"ßµ§í¿ärEb	àT¿æœ­äª9¿êðz¼^À€¿ïù¡¬'$¿ïïæ­H£UNASNone3FGL J1538.4-4656?Ò÷¥EÖ#?ōð}õä?ÅB^>¤«q?¿Ð/¾ð§Y?á3•ÍËê?ÅýÄL±Åœ?É?ºÍhJ?ŕÃôê€Å?Ù¬™¯¿'?Çè(=5ët?Ù³ˆê07?Ãk¯&w?ÜÈâ8z?²0"	?½F²køw?§^f½¤:Ý?ÙØz'9ËJ?±òM‡>Æ?¹Æ-ixGB?¢µ Vd?ÚÁKÇ 1ñ?¨:'ï_E?ÞÍ(ށ¼>?§-êk|?¾exw,?º/t•[Ïè?ƨ'•On8?¿€6¢î?æ'.ë>â?ÃLuž S?°Ñ½Q£™t?µ²ÍD?ßnX´2?ÌÞà*w¢Ï?Ü]8©®~r?Ê~P#?0~?Òý¡z}cr?°,ÒØÝ)?Ç»NöXº?°v×â½j}?à'[…Èèx?³–[Š`Ú?—_lëôVë?w\¹q&d?ßê¾öÜ{þ?±|¦A¦F.?ޟJ:-DÔ?±*×ñ£YMIXED4FGL J1538.2-6201?焻ž|,vÀåKþSýÀ:%™kvqÀ;&hI•u@dð9äRP@˜ þ?҆¨%M—c?ц^~e‹ ?úoŠfö¯?û:+õÒ*¿Õ<â^"o¼?ï£éIUпêoÞµ,¿çÒñ©ûçm¿é"µÏZEÇ¿ïó!ž¶9UNASNone?ã€/HJ¥?ÂåÚ¼ñÚÆ?Ž§çðQ§·?‡PŽÛR?Ø
b/±.È?ÂÔ)5at?áßƚϾ?Ä'H½€? Æšs]?œ76©Þ€ì?Ú'±€X?Ã/cG'n?ââ掍?°ò¨yÕZÅ?«Ëöœ«§ ?—ó‹£B×ï?ÖÂK_à÷b?°eRæPV?æu…'ô??¡9ù^ÆÌè?¸¬Îbu¬?"ÐyQ;8?ÊNÄç¯?œ_T!µõT?ÐiQÑ©_?¾ìCuC?£´
H®D¡?_{.­9?ærªŽ×?ÀT#Zo"•?ÑÉhÞT£_?ÃÍʖÅ1?°NUîŸ"?³#bDh›½?å€Ò½Ž?Śß«ÝÐ?ÖFí¼ÓÒÈ?±döM?¶q³êÒí? )`4'?âR¿?_?²NË\4^?Ý6¡Ðþ?¬Ìop*~g?ijhW4?¨ï…Þ²?Øp)9E'&?«ÊÕª*±;MIXED4FGL J1538.9+0425¿À)É¿žˆc@F
;:iÀ:Àß}©yÀ<dQüLY@E…x2Â@äG<Õs?Æ1'®ñp?·ßj‰5É?ððhGçö@(U+«u¿ïá) ¸FÙ?ïÓô©Š¨e¿àò¿¥œÝ¿êqðdx¿ÐgÔ$¯â±¿ïùÕ^kÆ"UNASNone?ïzåÿ£¹®?€:¢å•?Y(A0ñ?P¸ü²)õ¨?Ž!wó!b`?~òOÿb?ïÍ©4Ó?rZÝ8Ȧ?Li°ˆX?SVLßtù¶?uîå]ò?n,Ó´NÑ÷?ï*dîtÅØ?†-áyR|?v"
HÎ]?y¾cUúX?•¨Á¬h?_o¦$ó"?ïXëzќ.?p½;'#ôê?p؜4c¿Ú?\9=õS[?¬i+<?l~nGÖ§?îíBÌêe?'ÒZ6£?mÜΏ?fÂêЊÈÏ?žœœÃ6?û‰ô²'?ïVÉzTQ]?ß‡ˎ?a³›Ô~õ?gª[ÔT:?'ð]BÒk?	Y=K?îTtåè#?"
h}ªÁ-?"jÇQZe?lÞe??¥ÿØ-w3?×™± ܵ?îL«îӐ?Œ#w!¡DÇ?ƒ‰ÿÞë?vÿ¦l§zX?¦S€UX€?‰hCѵAGN4FGL J1539.1+1008?á3"ä}åÖ@G†Ð'}kfÀ:Ÿ9&A³À<WÛçl@3¡B/z@ÙÓËď?Å5 ÝD?±M…C÷&?èh¦è6µŸ?õËÂƹU?ïÿéà
v¿æùÕ
ãîR¿ëË>øcSŒ¿Ø7ÑþdõM¿çdßI® ¿ïÿæŸÜ©ºUNASNone?î g˜âÜÑ?©$¨Ê¥Í?oxˆ[:"§?ži¹arý?¤ýí<j%?£±džu?ï^ý͆í?—wˆÔx³?ƒXôs¾îZ?Š'?ÜzD?•§¦ø-4?b¢ly?íbÙתÔÞ?¡Ü៛%?ŠØþ·À?2}Çh?°Æ{±Ž‹?ŸÇbHÛ¢?î@=Í…?‡îIµ…ÒJ?™ùS8mL?€	Îz.?þó Ú§<?}ã…Ë?îyûˆeÙ?«¢8l¶•1?t'ƲÄq?~r*!¹$?«øtN—?ªeVã‡<?í+4æUxÇ?°ÏÞoπ7?šÛ»3VË?¢,§q×/h?¯ß08ÃE.?§.Rú}þì?ì¨ý*@N?¤Yä$o[?šL¾üRìú?"ÑŠxsÂ
?´$æí1¸?¡<·çô®?ê㯀œÙ¦?£ŠAñhÂÊ?´\OËRô? š|u%Ú?´†4/ÇÛ?˜š'üó AGN4FGL J1539.4-3323?ì'U&@1ˆ5ĊßÀ9(¼QT†jÀ<süQ×@ô$ª"N?øÿ0F祥?´þï3Ôî¯?ä']<ñøÖ@+‡_•'Í@æCÍ_CÝ¿ÓVºÂG¹?ïùgÁf?¾"–}/€¡¿ß';#l–¬¿íH>]2àþ¿ïéŸ
ç»UNASNone3FGL J1539.2-3324?'^lÛÂ&?‡Òrl=?ï_
÷0ðÛ?¨u¸;`ÍL?…¯#×f&ý?§5EÔà?™f68øÏG?°Y`'Ý?í2/'4ø/?»M£ÑÒS?°ù8õñ³?³š­*Þ	'?¨þ Ÿ
[?>N«oì?ê¦C]ö?°(¤tJ?¾…hŽx˜?®?ô\"Ȩ?'üýX93Ê?oLM#û?í÷þe'<?'JLšÜf}?«ÀÖÏyO?†Ô9
Š3?‰šµšÎo\?ö¨\bÓö?ïVÊ}ä¶?›45@ós?€²«:C0?‹07r‹wh?‹.™4]Ä?¡"¸ß/%?íã*	ù,?¶ÒÀÆË?«ÓËòñÊ?²Ù¶?¦QföŒˆ?ž:[>:A?êÌ»• nS?³øz@Í?¾qpI'ï£?²*iÂ~‹?m4òŽE4?_¥!ÇÙӅ?íÅ>õ¢ó¤?žÁ
DïÅ·?°ì`¿G#?ÚÍó;ÂPSR4FGL J1541.2-5201?湫–àña@rkݞ¬(À:×t¼j~úÀ<"K<¤@"QÂ$}@o$ù´Œ?Ög½ž±†u?ïÿV¢N@
ï×hE@ÀUE+Ù"?ïñ¦ ¿ç¿ì3	ý¯Ã¨¿À'åbšÔØ¿áäñ`®—¿î0¡™¹¿ÏèŸ{°ÐmUNASNone?ØT£?Â)ôä ¯?Íó"ôƒ?½·HãëïŸ?زt`ú?•µ€Í<V?Òò›ؼo?ÊÿË£h5°?̹[	!+?ö.Î.³?Þ°·qµ"º?ÆÀÑn¦G?å¨ö
/_á?±§Pôž©Í?¿"ƒìèc?¥²¬íï?ÉÊåÓJÌ?¬bI)ÍUt?Þâô^·?²:'&åpR?Õ·¨N¶?±¹6Ç+<?ÆÊÝϵú?©âÏN¤?ÍzÙç	?½òA.&6©?Ð_-"rIZ?‹fe¦Ò?àqèÿÍ?Ɲpüõè?¼p!ÕV¢é?Á¦;L9ó?ÒgO«Ž?Éýq dà'?ã>T8ˆÔó?Ê.[#"€?ß
⪍:n?´Û¾¿0?Èb­"§8­?°õe4µ?ÔÃÆÄ);?³ɂBúv?Ç"Ê<F#È?¯ŽÛ8ã[?à˜¢Î¡Ž0?¾\¶9bw?Ó=UD™Ñ½?º!ð¸ãMIXED4FGL J1542.1-5901¿ïZ¤˜?XÀÙÖ»cýÀ9H.Ä8©•À:èºÃµÌÖ@…‡°@ìJÆͯK?Äwøõt¶¶?ÂXȃ'ðX?þcˆÕü÷?û")ÿ°z¿à¢R‡"Ä?ïÿRü&V¬¿æÆ×Tæb¿ë®\Ÿ=H¿îÏp;Ñg?ÝßNdgÌUNASNone3FGL J1542.4-5911?Ü@¡l l?Ê~‰	Ú
?–ƒÖ—Y?—~àŽSH?á+•A£Â?ʳÉp"?ÙËE܋º<?ÄR=W¬í½?¯Gì'錞?§Çy‰€]?á%ÞITY?Ãiäóè£ ?Ø6Ïô¹>¿?³Ë‰¿|š??¹ÛvL§<^?¦OÄ•v¾?à©)<y?´9Ýúb*n?Ö]ʗ"Z?«KC¿*Ik?¿°»£s{ç?œ_ϒ\µú?àÛ]¦EÆÖ?«áðÄzx)?Ë
«ä4?ÀFΟςy?¦qÂç¥þó?¥ö&Þø.·?ç՝&¨¤?ÂVä0tD©?ōaìç?¼›5\û{?³÷£‹RÝ?²˜È@'Žµ?蟨CwñK?Á/
¬|Ã?͔‰u›H×?­
ý…¤?¾ýÖZHŒ?ª@g`LÌ?ä»"×V¤¹?²ªyåÄ÷^?Áœú³K-?¢JâÁª?ÇŒ~S)?­'E)¯ð¬?åòõ¡¾gk?°²qkåò²OTHER4FGL J1543.1+4209?¹N÷­Č@J1a¡Û‡À;s¤ÎóÀ<ݜûMé˜@ .ÝNûÖ?ý¼\!iT?Ïíþ÷ÂD?ÌqG€r+A?ý™s,Û@	¸vk5X¿åõí!Öê]?í¦¡‡N¾?çV)Ø@ž¿ãh³¦Äz¿Ú®ÏÁsÓ6¿äÁœýýtUNASNone?ïõÁ
 ë2?J-±AÊc7?/Âyúš¥?$K6q×|?P…œ¨gö³?F^S=§"?ïÚ@Àåbñ?qÔ =äf?CÚJäf?N	j>ù#Ï?p|d[—)?n£0å±»F?ï€*‰¢?'fŽí'm?d'¶3ôEW?l¾·àÕ`ü?ŠÚGéáv ?€êËE"©?ïÃC£1·¢?_Ì1`'
?R3Mƒç?Cn"š·y?yÑNŽCÕ6?\>Û^hF¸?ïåZRºj¨?f1 w¶pA?F§M£Ða?B¡'Á³¾²?dûٝõ,À?b¸;›Ž±?gM?Žk®é{Èè?V(åE'T?bS<þÛ?ŒúwÎðGä?Œ
`ò'?À?ï
Ò·ŒS?JÎâ$¤?qh¡»çKM?u°@Chc?šK€§LÞ?Ž.ÆBî1ä?ïp­<Â0Å?|ÑY*?]uýÃDÏÇ?X¸‡ç<Õ?øíT\?zÃR¬£AGN4FGL J1543.4-5925¿îx(]lAÈÀ3ý»'!®À:žlwø_"À;°ñ~\ý1@hwê@$9Ãp,¹?ß#v\}¯X?æQ­Dq@•%t-Ï?ûÍ%7G?ïùrz(¿íUâ_±?€ó;#Ë¿ãéošÂŽ…¿ïýn?΢¿Ý
v[Q	ˆUNASNone?Èí"
ZÔ?ÀÏqÅȪ?¬,qÁï?ªjoÒ¤<?è5=~æì?ÃKИ´Af?Ød_'À?ÈZ'¦=õb?©†œ»á;?©
)B§A
?â5ŒkÛ¬?ƍÐðjX0?Ý`Ï,gUé?²@s@µ?Á¿&ö'ÓÈ?¦ƒ¦ù-Ã?Ù¿X"À2?±Ó…•%?Ð?`ä­z]?¥ŒŸRn¡n?¶[ûð7[? Wô"¯?åÐç–?¬¿õ'Ã?¼fdæ+?¸''{~Uº?®H•l¤ž#?®®Ìñ/¹ž?ꎵüëg[?¿w_Öj?Á`¢u3Å?¾¨øÑÍE?±ä|ÿ ƒ?²©*ˆÏ"ç?鄺뵏?À`''["-?Ô¡gC[?±Ã";w)¡?Æþ‡¸y6U?¯¹Uj£^€?à5
^@Û?²ŽMÒoÕ?·c£€‡«¯?› ¾¢£¿ž?°ÞÐ z…?¥;Mˆô¶?ê÷±‹íxX?ªÍó¸OæhMIXED4FGL J1543.6-0244¿âªÄä÷ƒ@Cqà?pXÀ9òµ™ªaÀ<(P!Ô@$o¹Ì?@¥zxl"?ÂCK¯*ûV?Ûè]»Vƒ@`ûH
?önrtÈû¿á¤þ§R?ێÆ!7S¿áâP>ܵ¿éšïª/>¿î±±RóÂÛ¿ïÿ"	¶UNASNone3FGL J1543.5-0244?È?JÒ¥î€?¼38üö¶*?àüã¶]ß?É5÷9C(Û?Ñæ")_lD?Äp»$¿ä?¹\3'Ýl7?µN¢JNJ?êÉ¼Õ'u?¸‡®G)?²~˜-Ö?¥¬‡3Ž*?ϸ1¼Ts?°\ÎG'<ß?áâÁUË9?³OÆÆ0M?ÌmÈì~ª?¬–¡‡˜½?Íwí¢Z]o?¡7äõÍ?⟖Bn†é?ª¥ÿaÌ?È	¹Së†ï?¡"ìEçTˆ?·IßƲS?­}èHŠO¨?ãÐß at?ȧ‰Ç>˜?ҍfOÀ1´?ÄÎO»¡x®?§	!´'0é?©ï09ƒ¯M?ìMn•´Ý˜?·6
Ùâ}ò?²úyýHË?°lo_¡`?ÂÁ¸ž¹áZ?§¶éêÝô?ã'L‹sç?´z¤†PŸQ?Îõ3v'œ?±f&HÀÃ?¸JËXÃ?–÷åâïå0?åi´€b?²qåŽyOÙ?ΈšÌR1?®Ï1ÑFJPSR4FGL J1544.2-2554?åã)ÒÙ£—@6š€JœÜÀ9žµŒ>gDÀ<n5gÀÙ@"áÊà¹i@ÁµQà?»ï¨ïÍÙ?Øçz"0¤@ëOKD¢@Çÿ_¿ÛÒæÂAX¿Ô³7¥]È¿à`W=Ôvå¿è½¢B4­Ý¿íEK-û»Î¿ðUNASNone3FGL J1544.1-2555?¸ª\Ptï?³ž‹K"*?ë`ȊÑ]^?¼45hD?¨ž¾¯n;I?¨ÎEÅGw'?Í'*ѺÈ=?Ä,«¾¤ð?å×Ð=Ý?ŕ¬k°r?¶ó(oú}¤?ª¯°Fl?Æ^oŒÕ£?­—CnÝ?æ¡]³9~?²ÿu˜<à?Á#
ü³Df?¥¹ž(Áâ…?á[¬\¦r?§°OTQA?ÒrŸ<ÏFØ?¤ÄߤÁa?Ŭ£Ÿ
?™Ÿè8>C?§
¨î~ÖÓ?¤þ¸'=?ì÷¢%%˹?µ'à荞?©{4»´Ñ¢?©r§'ÑÊ?·	uC·?·ko•E>Q?êgæ%/Ü´?À50°ÄOó?µ·YËõͧ?°«n9ÎÀ³?±K¼ÏÇd?¡Ü©7&S?éæIy¬?­ÌBó¡v(?¿Ù¥´k=?¦	¾×I?Ò#ÖG…{?¨2£W?Ü:=ŠDp?°ï¢Õ¹w´?Ñ¡ìÝAÔ?¨NhY4î'MIXED4FGL J1544.9+3218?҇ŒËCÏ|@JÖÜGªÀ;Am
ÅUàÀ<Ç+w}@ ʛþ"Û!@%¸Që…?ÀˆÔº××ÿ³,†›»ý?ñ4XÖZë@ìU¿û??ïÿ?{@?¿íRŠ±ŸIÝ¿×M,Ù|Þ¿ßÖïEG²Ç¿Ê±"øu7¿æÒÎ8ݗUNASNone?ïÈ3Ž?«Ï8vŽÞ?RÖvr6Ï?K,Üe@?›™˜]}‹P?«Éœʆ?ïŽÀùB!?‡­áv¾R€?a"{!?e:ÀÙT?ˆWYù³š?"k%@®F?îÆ~À‹‡?"$S¦µt?_í¶‡R"™?YfâGh`p?¢˜¦?pi?"0ò§A?ï_/þþÖ¾?vw…¯?cuÛvLO?Nï$.ܛj?'«]>ßÆ?uòOfDì?î1ðzÑØO?ª#¤Ñ¯U[?e£²Xýî?]"®n^ù?«†½.UE/?©þ*îº4#?îî³®\Ž?ž¤)Ž›n?lBèlÄ?z5–$ó?ž§¸'Ämw?›l¯‡•Ö¯?í£w§4?ß=ÒCeM?cØû¬ ÁT?[ônñÛ?²Ezçàv
?¼Á÷ê?í£R÷¸wš?–±½§Àν?€œIvê`½?séZ_¼?°Ñߊò?–ª±¥ÑwAGN4FGL J1545.2-4553?Ô¤³ã
À'@O¿ZôBÀ9òóĈ[À;{<¤ËüÃ@U}£ôC@‹Äߘl?È9…‡¾Ð¶?Ԓ±êˆ@	¹JÚåª?ö³:9·±³?ï½!~TÛgå!I¿çši£1Èпå³À¶‰?¿ïþñ­VåÀ¿ïÔ'£]éUNASNone?Ò½#HÑÍ_?ÁÆL;S#z?®å®æŸì?¤"]	?äÀP2r?¦È
AÔX?Ð'žnYi?Âÿ¬Ïg—û?ÐÊJ{ú!o?ÁȪf¤…?ß!ä"¤j?À·Xs€ø…?Ý×S0~£?³e¸/_S?¶ñþ$ ?ŸÔ‹'WÌi?Ül"­†õ?³ÃIñY­?Ë2™sW;?›*Ç=''?Ø­ُË?¥ðºZñ1?ÚWuÿ¥V?£Ü'ß«º?Ânüº¾I?´#÷ɖ/®?¶Ø€¸ԁ?°2£¼^?è‰0ºKڎ?¼
pÅ©±®?´üÅꮫ?²"6å*£?ւ4ƎÍÁ?ÈSÚr§½I?â;æM¹ê?ÆsÖyÒ\Œ?Òíå£Tд?°†ó2'á?¿*oøü&?¥/õ'4Ü?⣿/UX!?²"xÿñÎ?­xáçÊ}?‰(·544þ?ßlTª¯Ê?¯¹Kø'Rœ?Üä3³@?­ùš~N˜MIXED4FGL J1545.5+2839¿¾G;]5@IÜ1&éxÕÀ<£3vOÀ=Ñö®H@¾d`QÏV@ª×DÁ?ÙfÀ=ó*°?ïÿøÞ£Žæ@
š;e0ÜA@®ˆ7q†U?иw?Ò}ç?ïÿÁeÖt?´Â9JúO¿ì†×6&-¿ïú™Ž±ß¿ïÿý±q&´UNASNone?éá€r£'ô?È.îË,í?™Îå?ÄUEÊÃè?§ƒàŠCæ4?°ªÎÉó?ܱ?9"u?ÌGf!Oº?Üm£Wñ•?˟#àôÐ?»"wY¹ëÛ?¯‡p¥™'?樖Q&?²[Ӊïp?œdÁu«©?­}M'íÉk?¿"ƒôÛx{?¥ˆ¥Ÿw¯?ᑄð¿ø?´ÍÛð k?Û"×Ž%??´–}ÿ@Z?›¡ñ>C-?D×è1?æPv2"ÛL?Ë9	YÂ?ÏÖ89
`?ɝÔãWäÕ?«Ÿ»öÕx²?¬‰–óö'&?Ó$WŒ¡€?Í
ɖ¦8þ?áÂøŽ$N?ϼ×ûî½&?«n®3"'?·Æòœƒó"?áÖk®Ç±?¸èH£
p?ÐGт`Y?·cÔ-"Á?È®@"b‰?®\ðÔ8?ÔÒº¢}Ä?¸ø
ߦ?äMvš?»¬fŒN~?®ŸåXÌÚ@?¢ÑõQa'¸MIXED4FGL J1546.8-3244?×}´†YöÁ@1¢ß"xîÀ:ÀoB­úzÀ<m¿Ü#å@ r"õ@ÓðØï?€"º•Ë?«éÃþr`?ì8é‹It¾@+2ËÚ3"?²b× ôÓb?ïöѵ(k¿Û_9áÎÅ¿å¡Äÿú¢¿à¬Ô>±·¿ÚàÏ6iIUNASNone?ï՞ZH Ù?gi(/´Ä?H2øØEà?=ÐÂq,	O?r0¬rõ¢ý?e%þփ©?ïÔâ¦0‰h?u¸¦¥ÊÃ?GÐLÏÿZ?R~/°ŠV?r"©-(Ð?r•Õµ»Ñ?ï¢e[ú?vŒ1ûEs6?[-8ᵟ"?_:nɈàê?"'Y8Ÿg?tØoAP2@?˜
Â?d×E«¼Ï?g+¢!ÕÌ?Kw¹ëMš?ˆ~'ò?cºeúá?ï°¢è!çÜ?r™®+:Û?^5~»<™ž?RêW•ÉÆ?€–%Eß³?pÿ€í;f?K2a?ŠJ'ñ—?[Ö1ÀŽp\?h@䲀Ë?ŠÕ§
‹Þå?‡åFJ¥?ïX:xÄ.e?'iõ«(
k?edÕÔ'Ë?e¹­Ü¬É¹?'L0qn?€èfãd?ý?îÀ­C3u<?Ë›J!úå?{íf,%>%?g掯RQ? w	Ïö?€Ùõê|YôAGN4FGL J1547.4-4802¿äÿëBâ0j@o'½†,À9 MÞ°$ À;lÀh:{ý@+Ý~uÒ@ø1jWX?Ã=ÛØ®Wl?Ә•=×@äZÏYo?ÿlå#/Úä¿Ö#fmG¿á'u=™¾ƒ¿ç|OÁß3¿æN-Š|Æ$¿ïþè=k›Z¿ÀsiN¿UNASNone?Ñ¢ã˜÷?»·×rB<»?Å7QOþÅî?µ³1Bê¢?áà¹ßñRú?À.ip˜)¾?Õåhp4y?ÁÚTƒÔ¥"?ÊÞGÛ½è?¹bÉØ3"Ó?Ü«É¡ì"?À«½ªèBì?Þ7QdC?²‹ÅÕéV?½ª·ARä1?¢êaÀáÈb?Ú^FÞGÜ?²Aå5"Û?Ú#S»­¯j?¤Ä³§ ¥?Ä´ß} «?š"¬D
˜f?ۂ<†Õ,ÿ?£þèȓȘ?À•½{Ã?¯Ÿ¢_Jo8?È÷wŒ9ÅÛ?¹Úo4Ñ»?圲¾-͙?¿ÆWNÐ?ÀWëæåÊ?¹~ŒÚƒ ?Ô¸n,9?ÄÌ͐8">?áöÏ:÷^?Å9çwñB?ÐSžÕJ?¯ç7.(?ÁðGZì?§œƒ¿ÔÖ?ãZ*ƒaHð?³»o_Ú?ÂzäžÊ?œ<yìG?Ð&Ÿ§Ù+?ªšòMÿ?ãNDÇ`ã?«Ç«Âê_€MIXED4FGL J1547.5-5130¿Ñê¡üax@÷RØҕÀ9C»€t.¦À:æ]	A@»¤"ÈŸA@ãO%AI?À8›Ñr?uကFv?¾=îß,‡?þ"jCk?ïþ•1U¢¿åX5`´ö—¿ë	¯Á¤$¸¿ÛŒ\å^>$¿ä8z?Œ1ý¿æ'zç&ë&UNASNone?Ï:Vèïî?ÄÚ4êþ€?ÀCw²Ø?'9åfè?çñé¾í]ˆ?Å#`¨ódø?ãr~Êá:B?Å'‡‰ÝË?–S8³¼	Ð?"±uÓ§—?×µÎÞÊÑ?Ä¡›ŒŸu?Ýü7Æ7SÌ?¶lç'°x?¢P8±X¾?"³ÇÏ)Kè?ß¹Á6?¶¹¸Pœƒ?ß&ÙÖy…?«(-¥×J?—½ÞŸ'?sê­J2ù†?ß]IÊyò?ªþÔØp*F?Á1::
˜?¸/÷ÎÀ?‡X¾Wõýv?…¨ûÃLžÔ?ëVX·Úªä?¹e9gYõ?Ô©`c9'¥?ÅrAjG`V?cêq^£5?¦lzÎ8˜ß?äÀ0zØI"?ÅéÜÊh:ô?Ðì[Ÿ?²Xf±Ãd¢?¤©?fËð?"¨nªŸÔ±?æ?^\#8â?³#iMIÕy?Í:½õðÕ?©ó¦l®5?¤¥´fñÈý?‡±b%H•Ä?çfõxί?«[¯¼	MIXED4FGL J1547.9+0445?íÛhý«£@E5@N¤©À:ôéË
TîÀ<K¢î¬ñe@頚¿´`@½¶°_¯?Î˔¨î÷?{þì.¼Öà?¯ ^¶ï–?ýŒ Ãås?ïl….¨‰÷¿ÛÜŸBÑ¿á‹Çêüó¿á­.l$‰¿ä¢àj8'þ¿áB£þøCUNASNone?ïwç8›6?›Ôd¸ê¬W?SÈó Šr_?O"%WÛ¡G?yYˆ2?›kU£'Õ?ïz䢬gÒ?…uœá¸òC?g>ìÁ4•?hðQÁ?‹w6"Q?'îãjK?ï*Ù´€"?…äCsã¡?jô•Œna?bôWË,‰?—dJÝgÝ[?"8ë<Ò(ä?î"K`ò?}ྜྷ'S&?|7U_¸ŒK?\¨U°Fë]?¤8С°£Ó?{'§Y0?ïˆ^;}7?˜KÉ\Hãñ?a…Æ÷ ]ø?Wá;ëÒÅ4?~;^ËS?—".1ókh?î±x´
£?ž'¥îî^
?t-
ˆ‹u±?{ea='?¢iæÇ¡t?›Û®&"ä?î%Œ_°zî?™낡XË?xceEK.?pT—óÛf9?ªšÍ_›^?—׬PŠÄÛ?ëèÄ¡Hÿ<?—­t
v£?Ž"y4Ëï?xѦV[?¼éZGÛG?–¡Ž¿ý¯¹AGN4FGL J1548.1-4416?ïŠp1sóö@Þá"Å&æÀ:‡0áI\À;Ã?¼®q˜@ËT‹rj@å"Ùîô??ÈýGéΐF?á]ŸîGq@Mý&0ì1@)ÓøEÃ?ìr>
þ¿ã
n}Œ¿âÅ~ú±âf¿ê "Êý¿´¿ï÷2œ4~¿ï 0âvdUNASNone?Õ^h"ðÀÐ?Àg·ƒSJð?Ì¢Ü\üt?¾ðS‡í?ÜP)=' ?ÂçÈ'¼?ϊҔÀt'?ÂñA°=cÒ?×.MìÙð?®'–s}?ÙHÈÆ­Ï?±Áùµ
>?Ú"Q¹Á?²Z'¨?ÏZŽä+?°`ág‡¥[?Ö~h¯Ô*?±xV9]?Ò÷>·"?? ¢ÿo'î?Ùio Zy¯?¥,‹/Ìá?ӟR)²DÐ?¢"¼¯÷"›?Ã}À	Åц?²þLŠÝ?ÒP}#ŸÊê?ÂXœí>ºÙ?áøQlH‰?ÃuX,øî?¸æuk¯)
?¹Þ¤Ì¹½¸?Þh~ÞF5³?ÉkÎ҂æœ?Û]ãÇ v©?ÈE;àù!?Îí´«ª?¯2hí[6?×ãH0¾?»IL¾äF?ÙéðB·ym?·øó¯*I?·46Ú°ÛÃ?'jg{/
n?á3Uqª?¯í–$?Ø&‹ŸÛÒú?¬Ÿ,šVœ´MIXED4FGL J1548.3-2411?׸ߗL.Ï@7DIDíoÛÀ:†Ôt`úíÀ;ú—t%kÊ@·É³å±@"º\‡À?ÒE3{W3?Ì
/Ä=Ý?øÌs@i|›@j£·Õš¿ìFX^»Í ?íªü-¨…¿ãçŠ$Óõ¿çP tοê%~>Ê@+¿ïû?ÏLÚUNASNone?ícqhðPØ?§±®'"Ú­?`<Èáš_?"hö•Bÿ?°Ìe"û8+?¥µ ."ÞÞ?ïzX§‹ö?ˆJ®AIàï?p¸—"éR?sª(²L?‰žØåž?…nn'Þ?ì´½¨ÜF?¢bãPÒw?œ5û¤ '9?'udÖÐN?³L"ÐñŽg?žÄ8D8@?í%žQ(*…?ˆždÉG ?"ӁÇ	«?q²íÍ«Hˆ?±Þ-Õm?…¥ÁQ5Ö?èÁ÷Ý­ÖÏ?¸§iÒ;?«½æQ? I²oŒ&€?Æ7_X¼?ó?µènº›?îdyžn?£ÆŸÈC?Š#ÞÚÕôË?"#hUx?£/ngó¡{?›ó0‰–´e?èB½0±?°*š?²®Ù8¬I?¡t•€²?ŝŸ$jdð?ª/¨Æ$•u?êmS¦¬c? ÔHÃÈ&?Ÿ¤}ð"õ?ˆ¢Í·èÀò?ýºôe˔?žÉe¢ÒAGN4FGL J1550.4-5354c?èU¿Xß®ë?ÌRó—罿À8}N€ÌCÀ9ú&	Ã@τ'Û9@ÊÄç%>?Ûqšânõ?Ì
>ðÛu@1bBë7@m%-O™?ïþ˜½?;?"¼ñ@'@¿èÇÚÄç%¿êë)CÆ(n¿àÞLÑë¿çÓÀì÷UNASNone<?Ó Ú¤ˆ~?ÅR:h l?ªƒ5YG&Ø?½‡x"Ì?äÇ_X2ϔ?Dz§4ш?¹›î*z?¸¨.Oý!?§"Æ{^w?¦)‡ßè_?ëT5Ó1Ñð?º£
¨òÊZ?ÁulË|¸?©'öêÁ;?Ä/\҂³?®b[Ü€?æ–ß6u¡²?±õ,CÁ%?¸%zò1ã?–ªK'?¢|ræS;?‹Æ‡ÔÄ>¾?ëÙhôá?›/Ìh§H?ǪAÙ$…,?À1(ªKÌ?ªîuz;Áˆ?µé
·ÕI?èfˆ2"?ÃÜÌx'âb?ªúK[Ú,˜?­ W
'õh?±©àvÁ?´ï±z_7`?ìJj~Æ?¸Ád"!9¢?¸³^ù ðo?¢?Y‡g?ÇÞp¡†U£?´¤°Ü¨Î?æñ÷ø…Éi?´éÏÆÍ…?œ1Éyü³T?"ÝQVE?ŸÃîޘÇÐ?—"â"y
!?î R=dw?™$ó™.(¡OTHER4FGL J1550.6+6027?æÔJUÊÉ@F‰"_ôöÀ:é5WСnÀ<ÒÝnÛî@ q¿ºëxß@³Y¼3øU?»__(R/¿³è‡UYh?ôý7Σg@¡Ë:¦o¿çxÂ
?©¢í\M¿ç›8 Z}û¿ÊžI—"ÆÔ¿ádãD–Í¿Ú4Ci\UUNASNone3FGL J1550.4+6027?ïÊK9~È?Bèe_Ž?EWYpáL?AVvàÑnš?x/x*'ð?5"›éZ?ïßêÛDxš?n(Qö.¨?@¡€ؐ?Iw`ο)?kìĕu?i…h•ÛÀü?ï|>€}u?ˆ	
qŒó	?R)|³?<j"D"˜v?Ž­º®>U?ˆZ>Lß?ïÐژí?YÀÅؾÕ?\¦.Oa?@õXê†û?p÷Œ_½‰r?XÁ@ω?ïÈjÙãâ?|ü^?M\áíwf?Cðt¸óer?x`jfaÇ?{^h]þ‹?ï"i¯¤¦q?ˆ—¬°$µ?Sm²,}®?\úÇF§	"?ˆ·óHwî?†¸*1	•ß?ï3r	v?Œk§.\Ó£?[XÔ¬w?[Ç$àhĽ?—Ü1…
dz?Œ
ï?ÿ¥?ï^ó3"ã?xT‹Â?x>Þwnk?dór¤Êf¡?Œ#Ãü"?v¿äÆh°AGN4FGL J1551.3-4920¿ë1ò_8N@
x¡Ú°»À9҃pbh«À;/Ÿ(NÓ£@s˜.4›¾@P¤þQª?Í×yär…Ù?ÁNÔäÉBÕ?ô…Őe?ûÍQ¤ãNÄ?ïøM·†ê¿Þ3LÉn¯¿êâѼÖ_¿âhá}V¿ïø¸BÒ¨?ïtã׫MUNASNone?ã3£Æ÷©M?ÃÊO bqË?ˆÝ®õµôû?‡"'oD?ØÑÊûêý?ÄJÕÑ'?äòAÈ;1s?ÅEŠ+p#Ý?¢¹P'3?¢ëp·.G??ÓÄZ¦gr?ÃmɑÙÜ«?ä.h•?²cƒ-jž?§Oánä?–¯b?Õ ùN#é?±—×&sÛe?âTeÀN9I?²1畼Dˆ? âªjÞVs?`ãÍ?Ù:ß2 ?²þf¾A?ÕL]É\?Ãî>êÿñE?›Õä'Ñ8?›õ㹦¾ì?äaª¯Áy2?ÄG°Ã¬½Ž?Ö*¢±×d<?É1vcé¬?²Iûá2@Œ?·qÝÚ9'‹?â¡o*҈ñ?É…¯4"?؆{ŽZ?²£:û;ø?²æý]ÍáV? 9)DÜxÈ?á_âB7!?³'IÙ®UÀ?ѹà‹ñe?³#/Nr	û?«Y\|š?"З»%¹?å¿
O¯üÄ?´¬Ú{'MIXED4FGL J1551.7-4257?§ÅÊÁX5@!*2	g‡ÏÀ9ԗt%kÊÀ;‹Ûz¹×@ššÊA¥@Úú—
s?Ãóâû¸G°?¸¹Š¿zîx?ô,byqÛå@ªëhÄ9«¿è4ÛϲZ¿áâ~
ÇÚ¿éGimO¿åÕ¥¹b¿å"&"À¿ïÿÀ	oëJUNASNone?êt?àâ?º+{Cm=?",>]?ž—¯-?Åzò¯?¹
{ã^Z?싗¹MF¸?¶mŒ>/?5•ˆ¯¾?…9.ªiK?¹|Ÿáý·?´ÿ»Ÿnhë?ë_ššÔ	á?¥u¸±k©?•ºÒ˜?‰WuY^Æ(?¿"v¦ò¿ó?£W­û…¿?í$è1#°×?
ޛÐWP?ƒp…';Wu?b\›D;.¯?´j­Æ<ÞÚ?‹cZ!Çkˆ?ã4eã4?ÁB?! [!?'…/á6i³?'
½mþ?ØȎ™á=?ÁûÂro£?çáìW	YÏ?Ʀ5–1Q©?–pSÉ,Ž'?¦B]ÜÁ?ͪD)Ùõ?ÅtÉBK ‡?ä')d
¬Í?²<ð^æ?ªn~ZEh6?—ôÔY²D?ӏÝl›ù_?±VnÕê?èxk&ºó?¤©%u&êó?›ÁEÑ°?}û»Z"?Ê®[6vM~?£«Í
dl'AGN4FGL J1551.9-6015¿ïÿZ¬QŠÀÀYÓpóˆÀ:lù¹"á¤À<
øç
¶@š>C\¡@÷ÀOæÈ?ÔðÍÝîÞ?ïÿÿÃw@zæ ³iN@Þȇî¡^?ïôž"|å?Æö©j(€¿éo`
+Òí¿ïôQ«Ä>‰?é©£½^ð¦¿íMt']è¾UNASNone?àXY@õ#ê?͐qó?Óµð\žça?ÎY×f®P?Ç2ºBí¡•?ÂgCñû?âf›"ž?ÉþžœôÔ? +?¥ç™?¤^¼"i…µ?Ù-ha•?ÇþPùþÅT?äxs1ƒŽH?²ï5©ƒg@?Æm!qû×
?®æéůö?DZÇõïÓ?ª÷Xˆ"?êȧyu?±B~NÙ?§—cmêh?¥¸®¡'`?¾3·¤˜%?¨°ÍH	éj?×Ô¦Ë[]Ÿ?ÊB…ð‰.V?Ö' ¬Ñb?ÌABÀnðy?ÒÈ÷Ðÿ?ÆB…‰tæå?ÐüúÜ4'?Ê32§5þ?¶‹ò¿ø}?À°E­‰;?ä°_é¨-?ÊynqÞÐÂ?àZ"ë•öÞ?µ[Ê"5?Ï˽Çå÷?²2Ù¢òS‡?Ïä"à>'?¯²Ô» V?ÛÃ{á!î?Å-äÐà¾Ø?ÉUz<Ôi?Ç*–'Zs$?בÃe´©"?«ßì°ÿMIXED4FGL J1553.8-5325e?ōÃ[?Ñ×r"eÀ6ˆËà=ÂÙÀ9‡‰Fe?@i9È£T@EüÁ‡m?ŸÊ
ª¸?»Q†'_8@¢l] l‡@©Ç "?ïÿÑa\w¿É_·
BÏ¿à-â@ÒX'¿âl"þª?"¿äžJÞÿâ-iànjAUNASNone3FGL J1554.4-5315c?'ï—êý@[?žÖ`Ù»pû?{´PûØ?}?†ZQgù#ó?ï1žß .?¡`Ý·Û?žžUŸÙÜ?§\þí2'W?Ûö[p,ý~?Èk²Dz@?áߟ?ÿR?Èⲉ¡÷.?²u«?¤ãz4	Ù?²!Ýi_çˆ?¤…ÍŒtÉÕ?ëiÁd0M?®‹}(ù8?Œìd‹¨'Å?u}Ô¶`Ó?¾¸5¢4ƒü?£ØMW£_?ëµG¹ÁÆù?¤òà(¡?™yÔ°°‡S?¥2™Õð?zCÝÞ²j?Œ$øoÙP?îÿ©žÒò?¨È…Ý}ˆ½?WvvŽXœ?—Ê}ò\?ÚöúÞ-n?Î)+-¼b?â$¶åý?ÎGȄ‹?¬3qúÏ?¡n±B–Œ?«âHz'Bg?¡¡{†ü7?ì~¤XÂíY?©ÎÀÂÓNÇ?t'¼}†º?cœî°ÈÅa?Á6'‡ÆLD?«1âÑÊL?ë‰5å%oa?«ûw0îGaOTHER4FGL J1554.2+2008¿áÿ/ÞȀ@Gäñ<îØÀ:³È±µRÀ<x úK‹@!x?×±W?ûQ¦&oÖ?ÁÆ£}sY?·KWí&ßh?÷zÀûÞ2P@I*-¦…¿ïÙ	Y¿ï@…3Ç-?ïùV˜"	]¿Õ\…ýZ‰8¿è•övêB)?ΗådsGUNASNone3FGL J1554.4+2010?ï´m4Î?¥	Ø?ƒ?RԌÌdµ?qÒ![«ˆ–?€Š)¿V??£L¦ïêõ\?ï"ùùD"È?M®Ü_ÿ?fá›ç?r\ØíÈ=?‰	æF[?Šƒ¤ïöä?ïDi‹Je?ˆKXé²(	?e¯_^äU?m²Ãt>'?"¼ÜˆºJÕ?†¶4øÍ¥?î,›H4;
?‰²¯S?u۠݀-H?h~Ÿ•v'5?ªz×`ÊQ:?ˆo~E³Æõ?ï<¤ 0L?ƒ™p¦qžr?bø[2¹
W?^Tûbìô2?‡òÀ!NÌo?'&y0t?èùJ§?¥vÜEß´æ?tô¦
—'?ô!>ƒ?¢h­¾i²¡?£è|µ³?î'ZÜ«£C?'ŽsöœÔâ?p4ÕHt?q)G€Ow?¤ÓÂ=à\ã?';º–>p?ëïnëΣ?¥'žEE?†Gì
§9E?'ü{^à?À"ÃoX?¤FÉAÊGAGN4FGL J1555.2+7103?ÅÕM™@Cš+<¼IÀ;
iŽÀ<å4W¡†@sgÇ9ï?þJÀ¾¡'?Òà!1H?ÞG^á™@h%ç}R?ý2xUQ@:¿ë64¥#:˜¿Ðô!:kH¿Þ¯_ÑvÖ¿åÑva†-¿ì´
(wîN¿ïüP}ÆÕ<UNASNone?îsñâ0a?™1'š,ä?'æ×Ê]¯ÿ?ˆ9EItãä?ŸšëèÁ«ú?'r¹$A#?ì1·	cxm?²ÿËs»¡r?°è¢ˆ?©­"ŸnL?¬Ì¾)ô?¡Ö¢f®Ã?ìÄy}ßÂ?¡…¤ìÀ?£U‡áD*?"tژH}÷?°1p GŸÜ?™fŽÎf4O?ì&iò?«š?•þ⒔"8?±%…$án—?…íÅ^Ò?«NVŠ›2?‡în
´3Û?ì<"üº·?©¥‹?cÃ?¦è'ö??›j¨VD?¯C´¶…¬‹?¡;ƒ9S?æñŽ«²~v?ÄB!(ªÕ<?Âó'ß³PÇ?À
û[«wh?ÁF3q'µc?´ŸÂÇs<?ê‰ oâ+?«š{SÏ?¬OæN&tK?˜óz'k ?½	]Kà~?¦$ø¸?èúؽŠ©?ª0?̔ZÐ?½ ¬P‰

?¥ÈÔtÕͤ?Ák¾tÅNÔ?¢¼—F>cúAGN4FGL J1556.4-6911¿å]¬R¦7"À'öº «qÀ:¶"ÿ®¡iÀ<qzØ
r¯@28EìžN@ðüõŠ?ÏcæÄŗN?ÙÙØN
O@¦ÝA‰?üŒcXÊÇ?Õ%ðál—?ïâàj8'þ¿Þ•¨sQ0t¿Úf('íמ 'ñ¿Ô×[œãUNASNone?ék)?z¥t?¾¹ïFìšë?¢•ÖÄê?˜¸—ꡏ?Å­å~Ò÷g?»IíÛvo?ê¤$åÆ!?¿Dw58?´·aâ"hm?±6½¼,¤J?¶(l÷ùA?µèÒNoá?ë=¥/­uL?¨)­¯mo?©LÑÔnc?˜WmO8ÍQ?¹‰0"\ð?¢'(]É;?è\ø%ë÷à?
©ËA¼¡?ÁÇh£œA?˜dâz*Šå?»¯ÿY|?'‹6ÅÝñî?ç[Z[–?Àߢì˜]ô?° N#˜nH?£þ´î&?ʂnð"½D?½Ûç`»›f?å†,CC»?ȍ>{–þ?Ç͓ŠûŠê?Ã@h60y×?øSÃ÷f(?ÀJ	ï$Š?çÅyê&ÏÎ?²FÐØí?²¹á¶ßg¿? &ȳ
úr?Ǎ'{%ì?¯4‡^ç?àòÂt{ŸU?ª¨¯¤,v?ÏÒãSï7Ó?­Î8MȀ?ÌbÚ"JÙ?¥n$4ÀAGN4FGL J1556.8-5242c¿âú
·WßT?áG›*½™À8ÐÎ{ùu¢À:Qqâ›k@ž>õ3HW@ ~ÅؼÅ?ÍÅrûË
?ÖZÚÂïI@
Ødà
—?ü…¤DBz?ïó…hŠ-¿á{%oü^¿äÇ QºÞ¿éÓ¡Ó#ÿ¿ëTu£KÜ¿ïÝ{¦i‹µUNASNone=?"ã²üÈç0?':dê`<ž?€•³{X$?¢è>¨!?ï‹™óþâ?–T¾¿l2?®Ôc"$î?²/rn¾kä?³©nßíÍ	?­"T,åׯ?띋êë'?·¾Äéù?µ]"w9¢'? ÛÖÙTÀX?µC+2dªo?¡
¦»ÚÐà?ê«öJõq²?§Ág¸ÒÃ'?•9b~?yäñÓå?°Ø_`LkÊ?jß(eN?í<I˜V?"‹çq—0®?"G"ŸôŸ?y°q¯??"±UÍçÔæ?…Æ~#þT2?ï\VUÂ?ŒqUÄôt?›ªÆˆR-ü?¡p{Yà¦?µšT -l?³,HÂÃ\×?쀁)hã?´êïb»?°k¥µ±¨.?–¾®×yˆ?´BŸ@ÈS3?ŸÝœí{?ëj7aC´?¤)½ìô°?u»îo=1Z?bë#Þ¯2ë?±÷ãõßõÜ?—b±ª?핋¤RI?˜'UDÛPOTHER4FGL J1557.2+3822¿b[-ÎÉiÿ@HåæFñVÀ;ôÅjüZÀ=ž¬(—@ TÜY×`?ýZ&6Ën(?Ö6ë¤~O?ËÍ&#€7É?õ	:q@ÿxÍFD]?í :}Ti?Ô¢˜[V¿âå¹ÏD¿¹u‰€-+¿êÇøð?ŠÈ-UΓ¡UNASNone?甆Q4aB?vm©ÜFå/?h6™Ö;œŸ?]Ïû?xÔ9?~"ŠoäÛ?r	±ó"6?ï•ÀAVÀ	?'\ÝߘN9?a­<àO~?fq¢¬Ø?†$ z1À?}°å‡¤?îïý]°¬¨?‰ðÅš?€ûýø€?ŠhWŽþ|?™'Åƺ?Š"Æō?ïpÙeËy?pÌG¼Ž-ƒ?vc´uŠ%?^õ'QÂ(?ˆ—Ì}7²?kžÅŠÞŸÄ?ïOâ<º_Q?‡"ï'ü–‹?{HcìÆ?sÞHå&r?Ž"ð©Æ™t?'£ñM§×?îïë®Ëk4?™s\ÂCt?qÔcca'1?~jºY'Î?qUaç?–Vɾº
^?î+fÞ[jŠ?–}fï36?‰ið‰•j‹?"ÆiT"?¦ïúw±¼?'ÓáíZç?îaԎb-ó?Ž1ì/j[&?ˆ`46à´?|¬|%焂?£Ê²ƒå±?ŠsŽÈÖAGN4FGL J1559.7-4518?݆>sV@nžÂÎFJÀ9¡Ä©èœ6À;ULf
 @¬3*úª@°#¾…â?ŹxǑúi?ŜçAm2³@ÅáõRþ?ù¢¾Úzà¿ìZÓÍ$á¿Ïߒâ›@8¿åÕí¨§c¿æÈÙ"E¥¿ìEÞ,ñ{¿ïúÿ?8$UNASNone?ݙ}Yòå?¿—þŽæ¸0?˜ëÀ¥C"J?'¯o¼ó£?àkãN!(Í?¿ÏRÁ¡~?Ý!jm7Ö?Âg( c*z?¹C¸¶K~?±D«-–?܍§µˆ"ì?ÀŽÞeâ™#?ä?[þ¤Ë?±Wf'\î«?©Ô»8è¹C?–?v£Ðs-?ÔF°0á?°E¸D¸=_?àÃ÷"Ê͙?¦vòŸ¡à?¶ï_ɜÀ?'2pQþ?ؼ9z~?¦øxìÍ?ÈíÇ'`0?´¼Kji?¦ÔÛo£?œ´ØÂ×ß?èWMÈq´?·1ܒ"ÕÒ?ÉeԔ±R?½Ò ¡J¾?Ã^«"Ü%ä?»Ü°‹šö?äÎßùœ°ó?Â\=e¹?Ø6°}ƒ/í?²ÉáfO?µ'hVc`Ž?Ÿ«&mÇe?á2Z¶x?³4["?с=s9CÕ?¨fŸ*À?Á¸l·cY?¢@¦ÝdH?âÑa+5…??­¥ÈÁMIXED4FGL J1600.4+0407¿Ôk=RhO@C¸ƒBÙÀ;	ð€0<À<€Ü…§tN@rX¡×«£?ÿd¢¬gÒw?Ïe»d°?ÈPIÄo0:?ùꁘñÓí@+´Ýí±t¿í‰Ú¿~°Š?ïÿVW$ª¿Ëú|]s¤¿Ú—8Á< Å¿ïÿÇËÜ?ïýjŸ>XUNASNone?ïhaG"‡?‡õºŠâº?+Eƒ}[?{Â2Ûpf?"¼'è±w	?€ð,°²š?ï¼M¹¤Ús?}íQƒ~šÓ?Xš)ó'¯8?eôͼÖÑ?{²˜¹·Ö¢?uJÊÖáÏB?îÛ²¥9?'ÇKJڃj?‡"‡§ŸY?‡²é{ù‡?˜À(ñC1?Œ9þïØÂ.?ïYÛÆV~?s
I7é"?q½¿¹€p?XÔ¢¡C?U{Ë1?p·"ÊØ;?îÐå¶'ÄÀ?—79t=?"«ïðó†?ŒƒYÜØB?'8GP=Þr?£Êq" ?ïA@<01÷?•TÇL;_?iM•/íý?víÔÁ"I?"®U€t‹k?'ÃgOù?î*…S€I€?™"ôÈ
²?°+d?9ËxšãŸ?¥k©‰`B^?"'9¡N~D?îMyœ	qª?;EN´[?¸KÍ=7?qv†Æ`}•?¦ºSH]"?T'›ø°AGN4FGL J1602.0-4402¿ãÞ
yxr@-Õ
ˆïþÀ9Ú|#g
UÀ;h¦Bˆ@§*ѺÈ@_tÝÛ?Ã|(ÚêœÁ?—Ì—ó§,)?Ùhm
&Ú@úã(-ñ€?ïÒ6™A¿áÂlÁÊ:K¿ìY …F%¿ÓÐ.`æt¿¿êŠ?åHD¿å³JEžpUNASNone?êá:Õ5sw?¿-Ƅ*¾è?z]£ûñs7?–¤¼ßÛ!˜?è'ñi?¾ú49?ë3yžÉђ?·G"@â(?vZØ0ê?|Ñ¬0þ+?ÂHÜ'?¶zÑ\r"?ëCÍnU?©€R_n0§?"Ӗ%Ø?É¹O õ?Á©D¡4?§œøwO·?í#t	£S?âüè]ñ?v‡K{ºõ?X4}]bâ?µx7=;ÇB?s£`£Ëû?åZCE$!r?Å彖pf½?•íš÷?Š¢V–îo?ÔIÀݗJ?ő°~JM?å–ÿÿ\ʏ?㚋©c^?î¦€Ð§z?Ž´²°´Û?ÔBŠÎ•?ÃïD3‹ž?æ¯AK¤Ä?µDrW­³N?£ëj ?šÉrérÕ?Ñ~äù6&?³þqøc?èeVI¸±?§<Ú®5h?'j¢˜î9^?yé""´År?Ì<nT`CP?¦ëÃùb®«AGN4FGL J1602.2+2305?åE8ãe.r@GoîN&ԀÀ:ß­z!.À<¯-‹S…¹@7ö'lO?ú½S,;d?ÌE}x%Ö~?åN•ÄøÂõ@˜u—5@ Žˆny?îE6̤¿é'ص8['?·SëåkÕ¿áçÁŲ§¿íB8¿d.~¿ïᐼ{UNASNone3FGL J1601.9+2306?ȉÈ7´?ÃX-†©…~?é4‡Fxy?Ä«z#©õª?˜ú¿Áyò?–ªèRb™?ËewÑÑL?ÂÒ}%o¦+?æ7Žš• ™?Ä保9aK?·x›Š²†?«±º2ýj?ϱb:T1'?±]¿Ÿ
ôZ?ä°ÝTѵâ?´¸ªF‰(?»PäÉî¡?¤A†û4ÓÂ?ߏWÜ_çÇ?¬†(²'N?ג)	°û,?®pÈ$¹3?Á¼þ3Þ:?š2Fy6"?Á&]ï–Ȧ?¸À–ònt?êI«LÊ^?¼ÐÙ̺ƒ?¦ËÓxn˜è? «ÜySƒ)?º6Ò¤ýü?º	Ÿ›Ò?éšvàuåÏ?Âåš4Z`Û?¹*õ®
?³	Úå¸X?NJ#|SZ?­‰‡q±š®?æuÿå«Ð?³9ðÖ[/À?½;¹ÙCíY?¦Åç®ý?Ѻ/çõ•?¯è·0z¾…?ÞÈY3«‡?·€Wd|°?Îû™ȽÉ?¬Ò¡|çÝMIXED4FGL J1603.0-4808?î&q26!ê@
ႁOùÀ9bžÕB½À:êæ0K!g@ìfOë$Ò@¿ãzŽ;˜?ÒLóc9‹<?Ôâ¿ù&È@Ù
By!T?ö>~À¨?ïûüР–ä¿âÝ|²ÙÀ¿éåïaLK¿è8«bnà¿íxrmæ¿~­C¼å›UNASNone?á‡"?‰Çƒ?Èp?5Ó!?´"{XèƒÊ?±Â íe'?×骖Ó'?Èì©û«?Øk`'þ?ŀÒ+)A?ÃL@¼Cù»?¹_øL?ÝîÖñ$?Ù>äÛü?وÖ
ì °?´+^ûf|Ý?ÄÆ´*¥¬3?°rôuœà?ÜÏßÀ‰6?´ÛMÊâ]?È0¶®IÌI?ŸÝÇ4Ì)?Ê1èÛK? ¶@¤wþp?ãlH|Æz?¥b§ò¦9á?Ü;,öGl?ÅoÔAhޙ?ÃÕ
µõ<?¾IOGn‡%?ÙÚMùÝüö?Ɵ‡ž‰1[?ÀDMs¡…?»ß["™¢?Ð|ԟ݉?Æc³|ê?㰂RÄâ·?ÆÏøVπÂ?Ïaæ¤å'7?®OÐé59þ?Ç?*$
Gß?´RU*õd*?âW»ÍÃd;?·í\€²¸'?ªãCúõ?ŒáPíwJ?Îh²AÂS]?¯î¥…M@×?淚›¢2o?¯tB`~DMIXED4FGL J1603.3-6010¿ÚNA‹)ƒ À̎ï¬.À9Í,Ñb¨À;ÿV?§µ¼@+~d	û?ýù™cé´d?ÁeFc¡?ÔÓXl¨ŸÇ@Ëï»@öצÅ|!?ïõ(5©/9¿}-©Ë.ÖÇ¿Ùä½ú¢É¿Úu»Ÿíq¿éõH·(ö™¿ë½¢yMUNASNone3FGL J1603.7-6011?ÈM֗ÑÃW?¶¾-ØÃ_˜?à['59?ëÒèUûp?Ó"Ə­â?¾Œ.÷å)?Í*pC´á?à —‹^?ÐÇ5|—3?Án€ÆäÖY?àQöÉ0Ç.?ÃÈÍ'ªWÇ?Õù¸·°Ê§?²g¢Ä™*<?ܵ›êúÚ?³²*ʃò=?Ê¡Vºªhý?«ÚF¾ŒÀ?à®]âø÷è?¢9\°ïœg?ÊR6óJÿœ?œã8ˆ­o,?Ñz(Àhb?ÄÞԗ´?º€¾ñÖ?ª)e(Hª†?áùIÃv?ÄV=ˆ\ì?ՇŒIW•q?Á¤\ZՕ?º•ý,æèØ?·"οd[)?Õ4Úsªê?ǵ¾íä?âÓ Ý?È`l'ÆTŸ?ÎÇç`ÌÉ?±h"†"Y?à÷¡Y4,?¶ZÚäSN?Í\‡":b…?¯X4ºëÐ}?ÑÓ?bbî?¢~xûÆ2Ê?Ò¾ñè±?«âæôÔj?Ûnqε–a?«=¯'g@ãMIXED4FGL J1603.6-0451?ìóþBÌ¿r@@ÒÒ¡øã¬À:<‰œÌTÀ<
Ê©Üݼ@3»QzF@ÆH@áqŸ?Å|ˆÑm?¸­z÷íâÇ?ò9,qx@fº¾'â?ҋ¢cAÄ¿ä'|^ö/¿ä‰}+¤É¿æ•ò—Ÿï¿èÒŠÝ>4¿ïýýâŽlUNASNone?îAmMÝÈ?¤ÍêXæÛ?~°î˜¤$+?xé'Åm'?¨
_[v?¢ÉߛQAÌ?ï}¦­dÚ?õhE8lL?k÷ßʊc?i½|õ…?‰˜Ž=L½?|
ú¬n[?îJrKï9+?•"	'©O?$

âØ?‰z]pš?£Ø¿c?»X÷ŒÖ?íñÒ+¹Ü?'¦ÃÞo—?.3,Ú?j·
áÓk?¨ËÄÚ¨3?~tkô-+?ë!*ö+s?³gŒì'F?•N¹ˆ²?ŠŽë`xË?Àђ'4Í?±õYzCÕ?îy[FÞÈ?›ÄKnŸ$?[N—þˆ?ƒeâ÷øDÙ?¢±–¥^ä?–áá«?ëåŠQÝé?¦˜wýßâ?¡?õ;|s?"tÙ@¯Ô?¸3²Ùx?¡I9Üyü?ê玍)§L?˜Þ>`Ï'å?¢p+ñ|Wà?"3 €eƒy?¿‹u²²?–æÒ}(AGN4FGL J1604.4-4927?à#‰A)7~@Àù²%À9:×ÑÍnÀ:¡²okÉ@18qÜf@26~AN?É
¢Gèø?Ӑ±þë-
@gȖÝ@=¨ø1TŒ?ïáâ"o?îƦ!è2.¿ãZ-þ•ò›¿èòbüO¿íRC™²Ä
¿ïýÚá¸lCUNASNone?Ör¨ Â?Äy¡*\ ?Ã:,:ŠYO?¸7/ #íã?ßðAÁ–bØ?ÅãbGjD9?ØÁX¶‹©?ˎbo'?Ãyx`}²ø?½¨©8ëPh?Þ+'x{š?Èï…Ëþ¾?ՇÍyps?±®²­Ø9?Â4ƃ#ƒ?¨¼ÀUÊL?à®çÁg5f?²1ó'ùoø?ÍÚ¹}`w?¥ƒå2LÃ?‰™
AfA? Õ­1 _?ãæë] ]ó?©m32)?ÍÁeVÆá?»ÖÞÍÅ	#?ÃIb8s'Ú?¸ôìG›²ê?ã½a"Q?ÂëŽ]?:?Ä¥XTR?Ã45'e[?ЋÑý/¸?È,Eæ
­Ð?âÒdbã>?Êùsš'¤?Í5¤îŒ?°òÉwuù?Áé€,A?©Ÿ¥|K~?ä8[–~²
?³<›qÆÌ?µ¿"ž?šÀîéþ?ÈJJ¾Œ'?­ú¼äÁBý?ç5‰™x?°)‡µ¦OTHER4FGL J1606.2-4602?¹%ˆP3-±@7 ÜïYÀÀ9üÒhAÀ;'²køvŸ@‡,ÓH@éi]'¬?×s]á~?ïÿ®2D¡@öà鳍@˗P=Ê?ïäžvx¿Ú'¿ó v¿é¥ø']<ò¿ïÿB€X*¿èt—1š­¿éØAŠäËUNASNone	?â
:¹öl•?É?!÷L?Åq8¡O?Â}±ËXr?Ñ,îEBV?ÅèΗ?Ï?n?ÆWgï¾r?Ô`M±þY&?ÈIIü^›þ?Ü'ÊûïÙ?Â`·ÕȐ?à…85üfB?²µ©'H?ÅÜkþMDÏ?®)Xhšö?ÔY"à'?±*Ri?Ái^•"¦? _¤ ö¿–?á§ßõôcj?³"ÑAëK­?ÓûÊh˜?¯Øq^¦¤P?Ù%£ä²X?ÈÝAm€?Õ¯_
ׄ?ÊÖ}V(;ð?ÑD{NCɝ?Åâ.?´Õhëi?¸˜ÃÎfùá?Þ6pÎãí?ÍX Cñ‹7?ܔ5/ü`Ó?Éhú.H¬†?ÖN"^
?±'ï]@Xþ?άDRQ?³¥w{}?Úá#‡ÌÐ?µxªÕ¯?šZØ·¾R?‡v(
UÍ?佶T˜ç ?½ÝgS5l?ÔÞåËmÉ?¼_´††MIXED4FGL J1608.4+0055?ï²É24@Bà~ZxòÀ:"€žP¸À<<g/ºï@lpÕ«Æ@)´Â&?Á">ï)?€» ¹Lé?ÁDŸ—4@Ì}EPC¿¦~ƒœ4Ý
¿áÄÁ/à˜\¿å?ÐÐgŒ¿é-=%$}¿ïˆ3
‡¶?ë2'¸#È\UNASNone?ï
îÜ}U'?£})¡d?h×õÏïNÔ?d^÷öˆëF?›'%·3XS?¢Ô	QïS8?ïp°T5;?Š•ðxÀ´z?mÁϧu_á?pöÊJßÜ?Œcw¶qm?…Tô¶ç+u?îÝ"]"?S2"tý?}ꈝfŽ?y.@¯‰Q?y¸5—?‹"˜ã6&Ë?ï3}6?5?wnä_Ë¢—?wNž3µKÀ?`Æfðé¦f?"Ì(Ì¢¼u?ràxW×æ²?íºuÉÓ²?«½±\FÖ?‡º¤šîG5?š§Üy÷?®iú>¦Ø?§ÂC'>‹?€Ù%Ã?¢UJ‡©%U?}Ô÷Ԑx!?ˆ [p7L?£œxøÌ?ž+©ûÕ?í§Ðð⚃?œ;ߚ¨äð?Šh´­ç?ÑŸEƒ?®èÃÅ´w
?™y8WÄ]?íƒ6£°8?–"Ù¬¨A?'0ßõÌÍ?qšö0¶f?¯4/b'H!?'~¢iÄ6AGN4FGL J1608.8-4803?ìõUš;U@"ÛÄ·UÀ9"¾®&˜À:¸Gõb@ÎfæÀ@—G½-óX@ëMý¹Ô£?ߛ9ÂC†è@ù¾$"]??úܔîZ¿àû	á€8¿ãr;ò•í¿çiŒöóçÄ¿ï8ÜÀ_×?ÕH߂\L¿ïù"–,ýUNASNone2FGL J1610.1-4808?ã=qñÆ®?͌­ÍÙT?ÃI1î݈?ÉØSÃí?ÏÁÓD?Ç´µºó—£?×Ph[;Ã?Õe8Ò7"Š?º$Ýɹ
è?ÈÔÀä-³å?á0´mA?ÔJÿ"Š¿?Ô.Ž¡Õ?²Ûûãщ?Êց%_¦?²Gñº¥ª_?ÞfŸÞÏ{?µ.t¡*é?ä]Iaç?Õ¬›K³™?z£luÛä—?¬GU㎴?ÖÚà#ŸJ?Õu¥RNEL?áùzŒ?˃Ä÷ãH?Ë«ï`—?É^€7Œ£?Ìn(B¥}9?Å3刎%?Ñô´'å	?Ӈx)v5?ŪråzÖ?ÐÜÊù/x¶?á›	FX\–?ÓÇ÷ƒ•:?ËNT'º"u?­GØ U?Ñ#¨Ò­ÈŒ?·Ñ8»_?àš–qúvÝ?·êmÞµ?â‰v±b8.?Ûô-ÏF#Ñ?•¢GŠ"?À2›;bà?ْòYº?۝‹£" ƒMIXED4FGL J1609.3-4326¿ì¤r‡ÿ5@c%}h
«À9ËǐíùÀ;[¦?šIÃ@	àÀõ~@ɎSë9Ÿ?øS"¢Ù´?ÚMú^ÖO@ŊžT~@zYWµ¯?ïÕ½Àƒ¿éÄ#°ß0}¿èb­ß¡»§¿çÜ$X¤ÜÄ¿ìFö£–¿—ß~øzòÝUNASNone	?멯pÿƒ?»×¢Jº…Å? ÿž»c?°<R3?ºkˆ#Ðiº?µóдÈP?å¾Òj4k?ÈÓsýJ:ƒ?¦ÃMÅv:q?­r{'V±?Ñ©ñr•ì?Å Ÿ'Ýs?çMjò]š?°š°»N ?²·ãý-!R?¢àm»?ÉncˆÄñ?­4e‡J4ø?é˜JAA¾¼?µ	&ëu[+?ƒµ[Q?yÇ?ŠOm֑)…?ÈcF]ÿ²?´G"æœïŸ?èMÙu/_?ÂsˆÿB?¸ÿ¬íæ Q?¾MvGs)?ÂHõ™Kã?·õWEy@e?ÚÇMf»ü?ÎúÁüÂ?ºy"êú¤?Áb"¦™?ޚQ^†7?Êý•f7?áÄ¡È<DT?´å»`ʸN?¿ò‰'îã+?«R]g[¦?Ôz	¸ÝÏ?²ëu,?áÏڂåDŠ?Í\m~³9?'˜Æfu8?«ˆjíëž?ÛFÁí˜Ø?Ìß¹Š½*MIXED4FGL J1609.6-4837?ï­ú‡˜@rï
åÀ9Ú'(böÀ:•V|
—˜@wh&"ùú@FxõŽ?Í2×XA	¶?д䣮…@ÆeÊÞ@[¤ÍOA¿ëLA³Ù?ïŸá§Oe¿çì×Ï_ND¿ë%5C®«¿äj)i…Õ—¿ïÿÿÊPËUNASNone?ã4HÓ>½?Èåc±¢œ?«†ûþ°Íý?ªª.«þºÊ?Ö&ŽÙï@?É4Š÷t?×$…æ‰ah?Ê
|Y0·?¿­§iL0?¼ôŒ¼2î?àx'ÉI?È5/íXˆ'?Ô"ˆ/0g?±¾ü˜G?Ã1ÙÆK´?©:¼2ƒ‡?á%¿JêE??²z§z:«8?ÒN……KÀ?¨R°èDìQ?¹ùãéš?™)ý3Ú¾v?ã´ÞA;?ª±|ÎÔ?â·§–SáK?ÆUƒC…ª"?°ÏFoÖ·?ªåÓª´?Ö\ß8# Û?Åàì¬u?ÄZ"zd¹Ø?Á!{Á¨'—?Í5$ÍÈRó?È=)M£™?㜭ô¼Í?ÊR'ôäÄ?ʕ3ìŸ-¶?¬8˄•~ì?ÅqÓƪãˆ?­´äÒÔE?ãþ>-{±?²¡Ö§Ê'i?½•Ð6c¿B? Âß	ѕ'?À‹Ô™
ÇX?§Eð×ÇfV?è*PÓy†¡?­o$,ÞoMIXED4FGL J1610.3-5154c¿Úž—Ùò¿Í@,ÀÓÀ8wSŸºEÀ:óøŠÀ¹@tœ…\JÚ@z–¹ëH¹?Å54?LÇ?×6a7R}@jaâs'?ᝄƒ:'¿îìñe2‰À?ïòË.g˜¿áõ³Á
&¿è§ØVmÊß¿íûW>«6z¿ïüD¿L±‰UNASNone%?©Ûn!Ú¿?¼w…Õcì†?ºÈÁˆ?Â÷è¸$?鳗ÍÒB?Ƈß4$í?–kî-)?¡À¶~»,?Ú´¤<b?ÅÃÀòׁ?áôº'²k?ÄÙ؁"rÇ?¸™!7}ݶ?¦Ð
¢2?̘²"Þ1à?°Ä4íD²?åƯ8+.q?³9
Ué\?fÉ3`b¿à?L!lJ\?Ó¬üp\+?­Ÿr°þch?æ¸"[—*?­¸Æ|é? –u'üÌ?¹ót°è§?Çh;›<?ÅXj$a?é0þ™3ÔT?Çw½2ÈK«?€>q'¯é"?‹9¿—Ĩ?Üÿþz;QÝ?Ìe'¡ìÏ?á?ýŠë?Ëõ¸8?²:¶Ø y?¡³C%þô?ÐN'Tóð?³Fç_¿?币õŸ:)?´/PlØZ?GWxE	Â?5!ÑV¥¾°?×#iA;?¶Çb§`Ö?ähu'ÜĚ?¶ËXŸdšðOTHER4FGL J1611.6-6013?Ó½8Ò{ÛÀ»<ĬlÛÀ:ïÁÄ[À;É°pçÊ@Ö)ax@@•sd{ª›?Ðã`¸vÔ?Ö£²A†24@hXJb?õq	̆+?ïû?¤Á¿ëž'ŒŒÁ¿ÚÝFA­ÊS¿æ¾Q€ž¡¿ëV8!ï¿ïøžý†¨üUNASNone?ÔÿíPÐÓ?Ág­ƒ†\Ñ?—\ýVäZ‹?ŽÀ¹‰µ?ä'n©Ò?Á¼Ç·ö7;?Ü`í²õ?Åzµpî2V?©µrO>0Ü?¥sïékð½?à42M@`Ô?ÄSÈö?ã
'Œ?²™må£ÂÄ?´+æ¨Í…?Ÿ6z":?ÔÙâ"äi?±UJÛgj?ޒ!\é\?£¸oÜQ'(?¾Àî«ÍV?"U'9Ë>2?Ù½ç¢ø#N?¤% ِëÐ?Å&â͕¶?µ
ùqSPö?¢A"Ò@hÌ?›¦_ÉÀÞ?é'5­«†?·pÞ}bý?ÈÛ®dà]?'qUå?´ˆ¯¨®ó9?µ™MõOyš?ç7þq_"¹?ĀÑٝZ?ٚo°¬†?²X3—Jù'?¼s®Á|•0?£øX·iH?ßH¥=ð..?³Fv%ÞýJ?Ï…£Ø?£ø®|£L?ÂfÀ©Rõ?£¹FQ•?ã¼E	ìµB?ª5ѯEäwMIXED4FGL J1611.9-5125c?µÜÕB7/¿¢ÀòyÌéÀ8$¹ØÔBÀ9Œûµîcö@xOE¤~@ŠQã!¢è?Âô`$-ó?×ÅäêÑ@"8]>Ÿx@\ÏRc$=¿Ï2¾°Õ?¬£"Šùï¿ãW榒¦`¿é'š¡×U½¿îûs®çŠ¿ïÿcøÍܗUNASNone4?a«9&Ù³?…ys56*¥?µå¹oêø?¹+ÊC#£ñ?ìýś³­Ë?¹ßÒ×"p?¢ÒÒŒ1O?¨úÒÂз¢?È×kD?º.¤`Ђí?èZå:?»ºAîY\?´Ý\úZcI?¥X²À	¯?ÍÎûoh?²O²wmA?å𕟗"
?´^9Ò¹¿¸?wf»7Yvª?_Ô¤ƒÎ?¸ÆŽlB]?—?=€ß¦~?ì¸`»ùã(?—ºŸ™P(?r4`®cN³?v>UýßÞ?³µ.KÇ?´ú7!Öô¬?ídñuüº?µ}‡î‹h?òh yô?–ܨMk¸?˼?@‡°?Á
¹ÞÕÛ6?è"l杼?À֚•h‡?¨8–º
55?˜ÚBbBmÍ?Ðfǻڦ?¶ÃŒ÷P­7?æIj0-Ê?·l@?Ud狗?Dko…¸?Àß3¿þÈ?¥HD/ßá?ë½£'.K ?¥[l@Ó¬POTHER4FGL J1612.1+1407¿í:åî»,@DÍÇ%ÃÞèÀ:†w-^À<ÂÛpÔ~r@Ü0Âë?ú†ØF}'Ó?ÇëX¦4]?æö·¢CC@¾1)?÷ä‡ÑÆÞ¿ïÿþøþ"?ïÿk»9ýR?»"òm›9¿âòq׳°œ¿ìÐ5½Q.Ç¿ïøœ>9¡ŒUNASNone3FGL J1611.9+1404?§¶Ïåyú"?±—ílzç?ìY&ôzTŸ?¾g'Ž[ÅE?±[`k–=?¶ÌC& m?²Eâ¦jó?¶jR+In"?ëÂ_ëšd½?¼'2Rk:i?¯Oۀ0÷K?§Y‰
å"?ÇÁF9}ئ?®ÆNjUšM?æªÞª3´?³È2šm:?¿à—²±?§/ÝÏd½Ö?ÇDh/hè?£VSç¼Dó?æá)c"<n?«"žÇs?ºmäŠÍ»?š¸½ï?¬¥øú1œÌ?³J6—€»?ìÔÀr\¥?¾ûæU_?°¾]TLr?µ§d례?Ÿ†væ·?¥fö©öü$?íEr
—?´¤¹ßêt?¬!U¥£èþ?«2mïÕb?ÀCÒ̯àG?©Ï¹ÿ$>Í?èR#GD?±ö¸'÷ø?¼ç>h›?¨I2 ?·Þ¾*·S?žßKäá¿Ä?è›Ä~îÑ?±ðă/?Âþ¡ÜT?©.à*\%ïPSR4FGL J1612.1-4526¿ìªGo]ä@5àqÅ?:À:"Ëùh6JÀ;ffÓs¯û@geÀy,g@Ý`#Up?Ùª\²½­?âH«4̐g@dϝ,@ 4¸ïJP?îÂOpV¿ä?3ÞLQ¿á'ˆô'¿é¹È®Zÿ¿ïý¸AûM¿ä²@Äì-»UNASNone	?ã‰;Ë­#?çÁFÿ?›ÿe32ã?"Ž˜¨Â?×-"¡‡ú‹?ÂՕÓçHN?á€õßHX?Áú/ÉÐ_?±±È'ù"©?©aÖ>?ؑ¢7UŠT?ÀK­}|?ãþŠ±Á¥õ?²æGÝý0I?´" ‰!ý+? -îuk?ÒúBz½¥+?±€"2¼Ç?Þ^@»d£ ?§Ô
\9?±½ü*ï~?û^‡T0?Ý2@9Vý?¨yÐn z<?Ò–©`rB?¼'³î¦Þž?¯6я‰ˆE?¥TD_\Z??å
ǒ·cj?¿•ßÙL–?Ð9ta7
Ä?Ў5Àß·?·k§¨?À(dÉ¿bg?ã5kú?Žá0 Ë?׶žŠøŸ—?³»I¿'!÷?ÀÀÆCÆ©G?§HG
ýæî?ßèþS$Å?´ÖVv£-?Éð·´HÞ?¤×TNܓ?´`Ê]@SÖ?¡D‡ýšB?æ÷¸ÇûN?«ÂpxD'MIXED4FGL J1612.4+0409¿æ·ÿÈøÜ@Bu"úÖËSÀ;Ÿ$`2À<±ÑtÒ9ô@ò§´i??ü¼˜6Ã
¬?϶ÊÂ["¶?Ø×@	,LÄÔ°Ç@+e¢F;?ïæ'j(¿âûjÚim'¿Ü&ŠwÔx¿ÑgïØÓÁ¿í
â18¿ïÿ›÷Aë]UNASNone?ïLp"ÃP?'¡A\*s'?…®8¨Œ'?ˆí¢¿e?‡ãIEV;ð?.Ûpå¬~?ï\wŽ¤@?‰ö"Kì¢?v÷*Þ?ycÿS¾¶7?ø"u,?7Ýë7õ?îaR—M?—ÛŽª©ì‹?"™ðªÃ$½?Ž—"ñ>:0?ŸEå'#¯?'QxÅBýœ?îP•a<¹?kæ¼
Õk?ò»½¾Ž‡?rÏO†?"?¢}J.|‰ ?{¶±ôق$?î§ìÙÁæ?œWñÐߣa?–bªñ»¸?"+}"LÐ?"Ÿ¹æŠ?‹!~š‡F?îVˆÊ‹ÌI?¦ëŸxeHW?Šþ¦n[?™ôª¹k?£×ñ±@? îÄ
´Î?í‡yè¾Ó?¡?…­Ò¬M?œp°úð]?"û"´£"?©P_}á™?™ù‰]%8ã?ë{Øݖ‹?¾5ƒj?£]s0uÔô?Z½uGÓõ?ºry\ã0?˜9+DÒBAGN4FGL J1612.4-4419¿îzŒåx_@MhÍJ¡À9êIHHn.À;7oE298@×ÆÎ0$5@üa'?ÕГÁ=w…?î÷‡ Q»@ً÷ðg?ü›è~Y!¿ïø罓ô¿?ïï"Áhj£¿ë/¿5_ˆ¿æúÖ?½/K¿Üõ™Ÿ£ÉÉ¿ëþ!²WVUNASNone?á{ˆÒ*?ÊßçXê'?¨ü÷ñjpI?¬òBQã?ÙêIãwÂ?ʱo·{Šn?Ê,ۈÚã?˳‰¥Ü´?Ø÷§	!oo?ÐæfµÛ]x?Ùñë1^>F?ÊЁ#ùPÜ?Þjõ^]и?²'\KuîE?À® '_û?¨ß¿‡ƒ±?Ù=ú__¿Œ?±Ï–¦2^?–3IÜׁ¾?z"j-Q?ìŠ2|¿?ºq[ÕòC?¹–Ûó ?¸øpñƧ?ÔÀôú	é/?ı9D*ƒ?Çþü'‹é?Á×@Än&?߇âPÜ?Èü·5
ú?±À.~6Ÿv?½î¤Ás†?áÊìÆÎlE?Ññ²¥?×ú҃ø?τÖ~|\È?Ӈ=óêo?°šªöƒí?È]°ÄG[ù?¯FHNè	?à$ôÕï$)?³ÌXfQ ?Q—÷³]¶?b}=Qßç?î-/Äz?· ¢Z/?¬¢'Oظò?¶¹Bßi*¾MIXED4FGL J1613.0-5102?Ý0þ# ²×?½ò6=Ô¢À7Ù¯ÅU	GÀ9Š¦V@~u@ªŠÀbÜ@r.þñG?¾Ì¡Ù¯l?Õb'|ñ˜3@¯ªŠ'¥a@ ¨²fD¿Ò[—?ø¡¿âG¦Ý¤áK¿à—à?ñ2¿è›U%ÌBc¿ìQ'[¶¿ïþ£^"_ôUNASNone?‰=KØ#?ŠK÷´³Ð?ØÌÉBØ·?Í"ÊL?ã3fi–qœ?Í; GK?«µäà·1Ò?´$«nÎ×Î?ÏF§·È{?Årx'ȝ?ær÷ÄGB4?Ç=ºé©#?µQL"#?¤©Ã˜y?ۂ6ƒAØ?·¿Ó§®ñ?ß)…i$ˀ?·ðDcQ÷?'žþÙ€7?hß…7§?µ–"‹(x?—E'J8ßû?í¿³Öh?—Ü°Å…/Õ?{Ø؞½ü?t|6_—}?Ùª¼ˆL^?Éãt¨üí?âòð
r'm?ÉëûuE–&?—+èåQëê?£F4z'"s?Ô®BX?1C?Ëä láC–?ä?Ëê¦ã•Li?¬ØˆcX˜\?ŸD'†Vg?݌ëÃ)'R?¼j*$@Á?ÞØ0OíÃ?¼5[èšCõ?_P¹ëŽ‹?MtìP>D?¾L‹\?¥OCT×?ì-Ž!QšŽ?¥*bŠ`WOTHER4FGL J1613.1-3840?×íAG¯'\@"$§Ös>¼À:°ðs›OÀ<
N‰Ðκ@ ø*$Á«\?óDJè[žŒ?áŽ-àc­?àÚ;ëh™G?þ1ßÈR@Ž¢ÛÔÊ?çZ,Ñð"<?ïxe!Aï¿ës…hŠ-?²(þ¦ä†¿Þ……zþ£ß¿å̂$2pUNASNone?ëqÐã˹?µÍj¾é?}êL>»à=?wHE=ʯr?ÁImz_u9?µ{y™B2Š?ê61n¦À?Ä­²Mª?|ÌB¶ t}?Ë†Ùw?Æ@Ø.Íh?ÃïZUáÞØ?ë®G`#?¦mÒIò?™çb±B[.?'bƒb2•£?¼ïèO?¤(^Ïp´?ì`u>N"?žz7;É?wÆ~aì^?m'‰¾Ju?»î.¾¦¼?Ÿ$g@ë}?æPN‰G^[?ÀéZ#YmÒ?–Œ\ÄjË?"š{j$N"?Ñö+ی>?À—prayö?ãܗj6Ìè?Îh¤Žëá?©ÛÚQ‡Â?Ÿö
p¨u?×Y'LöÓ±?Í*hǝ@¡?æ¬)
aß»?²y£=}?§—Î^ål?šüŠ4áŸ?Ïih2ˆ,N?°¬}»ÖÈ?éwÜ
‹›?²‡Ä…m¢!?xõ
+C¥?}ôß³Ùà?É`X/kþV?²—ÙËü»AGN4FGL J1615.3-1512?ëK¨R¢˜@8è"Ýz™úÀ:ŠŽ]%uÀ</j£	@­w'ÃiL?þ:‹KøüÖ?Òf';‡?Öó{!ßMÙ@f"f\Uk?ÿáJø÷£?æ'$óÅ¿æ´2ÝeK?çè?º*2Ù¿å6<!ÄJó¿âõ@S­&>¿ïþ¿UØUNASNone?ïÑm½À?"OTr̲?qò®€m?lN«Pÿ‹Œ?›)Lß¿‰;?'"ê¥~>?î庩¬?˜íûÞ¹q?‡tó>rù¿?‹Êq~xG?—Ž1)ÅU?ŽçÚFo/?íGüµëa?¡K‹ÈåPk?•t¦¡é?Gmóe¢M?°bð¨-·ò?œýÿ,—ùá?ê²8]®JÅ?¡>À '³×?˜?»±æOQ?"ÄüÒV­?Â/'œ? !'õ€Z?íù"èž©=?¢ýJúíJ?ƒ™ÿz\.?}}ï=,_?«€1—ì_(? w¹×ÉøT?ìñâçk_?³Ù Y)ë? q‰
NdF?¦Å"êí?°>Ôaw±k?«'7œ?êÔéy*ä/?ªâ­d&Æ?¡I/?"ûS‡Œ\â?ÀYöÁ45?§"n%2О?å÷u!6¨Ö?²°ÂÔF*ì?ž
ºcÖ£—?"¿ä"W'?Ò0j°VÜ?²yC)¶·ÖAGN4FGL J1615.5-5434¿ïÄÝ)¼<À¦°'ª¸À9á÷¯îpÀ;Fʨ/^'@Êx‰©@'ì®êc·?Çîüâê?ºd Ïª?ðxºvˆóY?õaDì³r?G)Š=¿éG1b"´á¿ã
'ž*x¿èVlˆ¿VÿáÁ*l»>¿ç+YnLUNASNone?ãÆey_?Ã''°RSñ?q愉µ?g‡§öžîE?ْٱŒªs?Ã"DGŒ<?ރëé-ç«?Ǐ3Xip?"yw8'Y?–è‹à—†¤?à">QR
Â?ÆÔ-¨R?âÁfKÛÃ?±—œ·ð?œ¹'°-Œ?žAtkA?ؼ§ÐúE?±=w÷hK?՞õæì?¤ñÙÎG^)?¤¿›[Ǚ5?…0Kí×Bù?ãäøNþW?¥=—$Ê9Ê?Ҟ·cŒŸê?¿v«Ô/?|"u+½Ö?q'çsû#?æx›'–Ðo?¿P9­‰?Èm1¶¡p?ÁÄSjÂA?™Ïû¸ˆø?¡öI'[ã¡?é;VÔ^M?Á±îšQûJ?Ôð›pUÊÚ?²UPV&Å?¥nVG?'"Uøu–1?ä0Ñf?²UƒlÀúZ?½…ô¡',•?š´Ê³© †?ª¦Už$ë2?"Õ<‰¨rÁ?ê¤ÜŠ*? ûë3ÅHWMIXED4FGL J1615.9-4322¿Â]VG_e@N0DkjÀ:"A±{7¯À;jÃwï%@ÀØ#B$h@8Omü]?ûéM¼KuI?εN+>?úzDºD4@ÜCR:4"?ïb<jêY¦¿ß	?"OZ†¿ë'ñ¡îQØ¿æn~ãµÇ¿Ø°†zØä2¿êƒËf›?ŒUNASNone?݀ƒ±Ð?Èù»~÷?¹ì¤áÿÂv?òǃóÑ/?ÜS¿Î?F?È8øM"?äÿ§Ð
'K?ÊԘPÌÔ¸?›hÀº™F?£³ßE>[W?ÔJ$T%Ϧ?ÈÁƒÇÉ¥?åM{ïö¯?¯'ªµbÝL?«´yÆtÖÝ?œß 
¸Dô?ъÕψq‡?®%0
w?ì8iû"¬?®µ! Z²?X™Â9òÿ4?eû*´ò…?½ÜÕ¥Û¾¥?®uò‹W?Ñgýó¾Ý?Âÿƒ†©í?¿Í¶íÌ?ÅáûÞ]?ãx#cîx?È''c?Üûì7?Î\_5‰hŽ?¬ßëº- ?¸ÂÀm¦ž%?߃{uW…?ËTeCÕ?Ü]ƒu¸5]?²Ñf@zQ?»S
‡ì·¾?§É€½Úµ{?Ü͹)_}r?²•Ã´ëǞ?æۉހÌ?Ëy"ŠC?máq+Št?"o€Íb!r?Ò
+¥Rèä?Ë%±·¿ì·MIXED4FGL J1616.6-5341¿ê@É)1Û"À[!f'À9]ħd]À;Ùô¦/ª@@§.­'@›Ç »aj?À7™NÆ?ïLùx&'K@!Í¥¹bŒ½@Ô+Ž#CÒ?ïäiÁºŸú¿Ýƒÿ°É¿½¼dãoü¿èŽ?{¿î(ÀþãJh¿ïÿUJÃUNASNone3FGL J1616.8-5343?S‹7¥å‹?ZÍtom?ï0²›PÜ?ž£rô.ߓ?˜·V<#|?h1÷Ý?‰L¥ËCó?"(´Éº[?èv`Y‡?À ¬à?¾?Î9\!éß­?¿tG~Þq)?§XeýÍÛ?™)mÊyYŠ?é­<ËÚ«Õ?®ûºÍ¦#†?ÃtóQÆÇ$?«ˆÉ#á5Ù?zÙ9mcš?b.\x¼Ø?íluÎ.w?¾\Ö÷q\?²îÃä
3¯?cMåã‹?Z·ˆ_þ?c§/ŠðQ?î÷áKño?¤èu1¸è?ŸX]ö;—A?£òbŸ¼±<?~\'Û?þ\?‡fðl<¨Î?èUÆ[/§?ÕçC¬¹B?Ͷóqɓ?ÃT¼…='?›ŠIlh?µ±"L?립æÍK?¬…žÅî?Àˆܙ7c?ªÎj'?KYÔ1JБ??,xä·Ó?îFóݧ?œÁÍ«Ÿ¡?«#ZàÉ?œŽ´ºç"úPSR4FGL J1616.6-5009?ïêÃQgÀr?×ٜSˆ=QÀ8LÀ½ÊÑJÀ9ÍLê"]ð@ À‹–!@ë|þX`?ÉtAEo Í?á3Ï@ŠÎ-±ê?ò!#"'Ä?ËXòŠv'¿Ùµl]÷,¿äM: ºË¿ìZŸ2ਿíTi¿n¿ç˜Þˆ¶óUNASNone?¸´a<£!í?À¥ªF?ÌJ½À•\?Ê¡5¸QHP?åÖÌiiië?Ìß×÷"`Ó?§ú	âP?®°løYv?Óä¿T5®°?Â+_Rø²?䛾Æ`c?Á—.߀G}?¿Ê!KÕœ?¨ü¨l!9¬?ÑCª?Òö?²éÉÙэ¿?ãdæ•åsÑ?´^ßFg'?gVŠuL9?NùNðŽ´Ê?Ξ+iI?©<IZ²–$?èAµ;¥a?©eÉ£ñŽ?§'Uî´û?Á"-6ømB?Ðþ'sڏ¥?ÌÅvPX í?æ™fÃÙ^?ϓÀá0?‰{¹‰ÎöH?"h]Ïx—?ÖÏ¥{·ÿ?ÇçOæ?ä2>XÖ/ø?Ç°
/"ÿ?´Æë	Ä?¢¹#¬d?Òá&ÑP??µ®V©¢?äþˆS?¶§spé?BÓWj¸Z"?1'¦Â"µM?Òß`Š{»Û?³¬s7›|è?拚åùQ?³±7$lavOTHER4FGL J1617.8-4418¿àûÌÉ¿¯@­ò>v]TÀ9é:G#«À;všÛ¸ù@9(_D´@=˜¿p?×è^"Ë?ïþ©SK¯@ÿSŸºE@£ñ~Ý֊?ÜÄF€íÑ)¿ÔùQ$µÁî¿êQˆÞ¶YC¿ïþð g?ï(J®kc¿ïý¬2ùQUNASNone?ڪϭ¸ñŠ?É
?i…!?Ð!ˆ'èI¢?ÈÔr U?Õ3§Ï^ÄÔ?ÆÓZG@¨´?ág,6¿¯®?̲èí¿·?°é½çì3?µŒ+H¸i?Ø÷e£Y7?ÉéZ÷óA?Þïc·×¿'?³i@"÷vÍ?ÌI	",j?³ɺq÷?Ó
w×*:?°½§\¼Ç?å®z'8˜?»Vj.-K?¡èóGU—?¡Èe‹ªUš?Òeìtn".?¹@½MgŒ¸?ÑDïDGå?ÅÕ¬:?ÛõÌÒÎeö?Ïkìçc?Ú?ÒÅCé0R%?ÇÈ[¹d:<?ÑC£M¢u5?Ë}ìÈsTi?Écî²$ÕÍ?Ë]iŽJAS?á2­/Q?ˋ½O££«?ÔBžBI?³ŒK:Ī?ÔÈBšÀq[?¾¢4®ï}b?Öõ"dÒ?·€æúå(?Ñ–Y¦Ã?Á5ÀLG?½Ë¦ºœý?À%øº2ã¤?ãÀ¿ûOŽ€?á+H$©MIXED4FGL J1618.0-5119?çÞڇËf¿ä3™Š€!#À8aOZ±&~À:`ÇÀôQ@ ®¤¸Üó@¢ñÄÓÚ?Ä©ò­1&?¹UJ4VžÈ?ü­ÚB×@›cÇЎ£?êÐxR÷ô™?èD
úú?Èrè•U<H¿åe»¡k5¿éDù>oÒK¿ØøÒy´÷ÄUNASNone?£S´xÿ+?š+KA?'ø²·UtÚ?"¨^¼?î;	/B|–?¢"Ó¾B¾?ºÅŒ‰G"?¹†Ùt6Cð?«=yÖWPy?¨
eÉäè?êóvч`v?¼M²æFÆ?´cáƒ(™?¡ÖJgâ?¼Ç>dáùQ?«âÞ(Œ3?éڜ^âÂ?¯ ð>í?ºd¹èïm6?ŸÐ0Ü 9Í?§¸ôiÿ
'?'íù©_ñh?ë7Ù|æg?£¼ÿöÖò§?— á'öß³?‹¿MT¾ë…?"µ[‡"&?•
@«!ôu?î¡Lsÿ‰Á?#÷ñ,?¯˜ØãV?¯—d`&Ü8?°BXb×5'?µcÜDÀÎ?ëþ'et£ì?º9Òt+ î?¯C²)¢*?š÷˃?ž?¼Ùlû"m
?«ÑÔ`¤ar?êp¡¥y<?¯tÈP|ŸW?¥×q$1Aÿ?"'u¦è>?ªÿÐi¥»?žp¾'DFê?ìòðߌÔ?£Ž¤$
lOTHER4FGL J1618.3-4537¿ï«¨¥ƒ»@RÍÀÓgÀ9Úl <K
À:#ÍbôÁÞ@渭Ûð×@ݺZÚA@m">5ŵ?âm-êñÑ@»†Eÿ¾'@¾n¢Ÿþ?à‹)ßwtV?Ú÷;ÀöTÛ¿ê±­ÿ"Z¿ìaÄ@6Põ¿Ñ/AÁÁUö¿à3½Ò^FUNASNone? H:ˆ:lP?¥tZhè]?°"ì=ŸU˜?ÅgE©?ìêÞÏÈnˆ?Ÿt%@×6?â¯ß}öÈ@?Ðîç?¦Š‹%P?²°DI
Ö?×à³u?ÎéÁF©)&?Økrt'¢T?³!œ)¾?Âsè¿
†0?¬;æz¼Âe?ÞZ™*Ö9Õ?³=è¥=?ÕÙ
ó£ü?Å?Ɛ-ñ;?C•2Èãód?bƒ*½#ÿ'?åq.-ºÎH?ÅKYýn͋? ¾3ÎQK?¤kÀ Ÿ?¨,yã?µDß,³­»?îÛmhR?¸g‹—‡Íh?Ùù¡IÄÍ­?ÐÔg)ž£³?¶"E_r»»?ĈØÛg´?à2¦¯="?ÏŒ‹‹†S?Õ,¶½ýã+?²B?‹¶K?ÄÛí$
Ùæ?­'$
@?à2©Wý—ñ?´bÒÄCÍ?Ñw'㸐o?ÎTB2»¥C?Q:í^453?~døáÖYË?ç;Ηt®?ÎJöòèˆMIXED4FGL J1619.3-5047?ï[±V7
¿Ø¸"*}ØÀ8¡.¢ªºÀ:¸ÒD@ƒ8XŒ@x@@aïß?Ë"">Ä6?Û²Çë¼|@®ˆã—?öþJ«ŸÖu?ÖîøüU¦{¿ålÿ!³®ï¿ÜkñUBQ´¿ç…`'¿í«a­šž¿ïrBþx%UNASNone2FGL J1619.7-5040c?pƒŠ^tG?}ÇûŸ?¨‰§KBzw?¥ûÌÉï8?íóánøä¶?¨½½ì-fö?°ivJE?±ÂÏ»ùÍ?Ȉøí<.?¹Ú3}0z?çСAs?¹é$åEG;?µ­PŠÐá¬?¤
¶è4m?Ç
°ó}e±?®*­ïæ" ?燩±â>?±ú³Å&×?~Js±r':?bsûĖÑ?Âç-˜‹õ? Ð~EàX?ë#qM}?¡-uAì µ?€±<_Ä3?z‰§nþjF?¬
˜çñU?¨Vœ9Ÿ?íü'€<óž?©Z8_áʲ?"ÞÝy ?šºÎ&ü߈?ÍëÄý©B?Âzó/<?çäwÉ?Áÿ-÷T?­o"÷ïs?›.Bï¤ú1?É󻻤Ӭ?³Ž›
áD#?ç¬ÁEb¾?´=¤ÔŸÏË?\ßi¡¶?HvÌÆlp?Ņ™Á\¬?¨×½ºn?ꐻwöíÄ?¨ìk"ÈOTHER4FGL J1619.4-5106c?í:ôû•A¿ã°™?׆dÀ8=³/lÕÀ9×Ô)¸`.@!GÁntÒ»@'PǙ?Ñ
\^ûŽ?À½y]9!@^aµ&¾?ý|V[?ïÿúŒ"¸'¿ãP'7§¿ê"qh"¿ådÀÉß2¿åҗ¢¡§¿ç®ÿ\lUNASNone$?¥e<CøC?ª¦ã,?~IN7Ñiž?¡ANÒ;š¸?îmŸt‹(?°pkë|'?¦ïÖuIJŠ?¯C^K%G?°¿T¸A=?¯dœqÍ·?ìy5è?¶w¥.÷Z?¶c
óžøÈ?¤C‰Æׄ%?¹{
-…"5?¨Ú2`ÜV?ê<üh@?¯5°gÆ ©?'Áx¦qþ§?t¾!f¹ß?§"ÔÑ 1?[w
íBR?í÷Æú6"¸?'E9™I€?±s7»?¹NTó]–o?'å61‰Ÿ¯?¢ÝÍÁ	*?í†
€.?»Ç45Öjt?™Ç³O¦›?¡ðãíШz?·¹:PŒI?¹gM/øZ?ì:›qB?º—`*q?´Szâ†?¡Þ.ç!¡`?¸N+1Ÿæ?§þÓ&¥} ?êtØOj?¬I2†?r8뎘Üs?_xy?¨-Gö^£?œFqP½?îZ›TYÉu?œ\%nPCOTHER4FGL J1619.5-5014c?ïn±Stœ4¿"ˆ&ÌêÌÀ8ȽÇvK·À9»òt&BŠ@ÚhŸ{°Ð@cnda©h?ʺðViÄ?И¹à6*@
Þ ²'/@%'~È2¿ïH¤´Îí?î<|½ÀÀO¿ØbO §)û¿ä†ÞvB||¿ê™XÌIð¿çï7@-ÌUNASNone3FGL J1619.0-5014c4?¹õ؅xáy?¹(:¿k&?¦G~w\á?¦´›ÖX•?ë`@win?¾Tæ2	Μ?¹­åßuúa?ºÝMAvö?±3¯P'Qé?±/'îùt*?ê£ÍYåy—?¾0´ÜHÉP?ÂrdlU?©HÄùpy"?Å´5öbP?­]¤t3Ɛ?åöm¼éLW?±<첀?§à†Àˆw²?"L¶N÷ƒ?—µ#¶é?€ñA'm?íÄO"°Œ®?˜îñQöɟ?¦"¿˜gݍ?±ÐµWþå? žÂüœý? x?ó.7*?í"ê*€²?´yþ
~Öl?«¼Y÷"?¬*ê6ۂt?ºó+8ñkÆ?¾žÎ{'a[?êåÔùŸœF?Àbx‡Èƒ3?¹	`#Ͼ?¢,"'Ü'?ÅØÀËn?°e-Ž®"?çhÏ˕ü<?±ÆwN9J¯?'QI'¨á?ƒ£gq%ùŽ?›ì$ÊÈbE?—5¥Ï?O&-ç?•?XöàH_OTHER4FGL J1620.5-5729?¹\žÈÞNÀAÄÆnÀ9ßÊKM
À;‰%Þ¶Ú@
œß^@†{¯£Ç?ÈP‰°B}?Ægv[Ñâá?ÿòŸ	E# ?ÿUûƒ¯?ïˆ&_e@L¿Ô
£\ú¿æ†Ž¾`¿è"Ø¿Ÿ<Ç¿éâ<›<¿ïþØ
bUNASNone?ݎÃDìKÌ?¿…¢"̀?'ué«V?'†Øx.ìN?à¬õÖJ=Ö?¿œ£©ى?âmÔrFR?¿É9/?–±6­.C?-·r?Ù¹C³^×?¿tíEpÖ
?åô­'&EË?¯Q™$Ô ¬?¡¾4³¯Ó?Œ$¸l?ÑôÍë8{O?­øÖÚ>f?åZØåE$Þ?œmCzS-O?± ZŽºð?"køÕËðJ?Ñ7'«}a?™ˆ™)!Ût?ˍ°hyL?¶ðÙ}'x?˜®…þ ô?‰·áb˜ìð?èrècðÚ?·åÀ}	ö6?хâ³úÿ÷?Àk9$õéã?¤©Áü"è?¦M·"'"ä?åòr"®3–?Áyn":è'?ÙºñUöµ1?²Ñ%úN¿?­ÌŠFeK?•ú¡ðuá?áIªŒ
Ès?³=@(Ä?Øý2ž?£–u}ԘÓ?¾+íÚ
¨	?—øˆ‹d?ßwópic`?£³oûìÔMIXED4FGL J1620.8-4958c?ëzî­¿Á?k'Úæ@À8s¼W3Ã|À9¤2ðîE@ÁÔKòç@Gòš¼¯H?Å2"{€ê?Ѫ¿±±=@€Âa8ÿü?ÿÕ©$|>¿î/§íå?ïoÑÿ¼Ž;¿â=à‹F¿ç˜§Å¬G¿ê–±‡Ìè¿èÈÔð‡½UNASNone0?u4%ãÊ®O?vxByÔ¯©?5>?µ"?•¥i—¯oÖ?ï`»&O?˜Œ\œÍ?¬°|¸vú>?²—kœ$F-?À²î<¼§n?ºzà±Óo?ê<¤öïá?¾Oû­Ý?²Áî…*ã? d»dœA'?ÃÒEñü²?©ÙB¼h%®?è³<ù¡R?®a¨ópþÚ?Œhö{¬O¨?vè"w&?¨rtÃtª?$'nrƒ?î4ٕKñ?'Ê¿qé~?zñp넃Â?œÀJ×k?€º.øV?¢tó¢¥5?îÞLo;Ä?¨m˜OeŌ?˜¢O!…ž«? W-8Þ?Å©hàzdÜ?Á©°Vä,?éГNâøD?Á×}»ÿ?ªb¬cJÓ?"@çÖÝT¬?Ä!ø×0˜?«ül¾¢Æ?éQœ§ÿ-?®1JúÄ?rŒÛ¸P~?dgÑ¢(ò-?­€¹ifÎ?›¥fý;s?îàÚö±"?œéf	çØOTHER4FGL J1620.8-5035c?ïÒæ¾Eõ¿Ú¦lü,¶ÂÀ8A˜iòÀ9Ð1T5â:@!
"é3_Ô@¥ŒÄŸâ?É+å¶þ"?¾bcL€Œ,@Œ$›À»G@¨³Åê°c?嘱…K.?ÏÌ
…&¿æë%(®u¿æÆÕ½â¿æ5þßÄv<¿æU‡Ô>UNASNone4?³¶¾|(ÏÀ?±Èe)½x"?ˆ0sÂÞ?¡Ý‰~§©?í&çntãé?´1ï<«…i?¨hHhÏwL?®@'ÍJ ?²çÌY>É?°ÏP‰Ö1?ì6~€Úr?¶ë´Ø/¬?°€AZ˜G?žÃš61T?¸Ì—¢èZ™?¨Q+Ԋªj?êÖdàGä?­f—!ßÁ? çØ­/íf?€¹W×Ü»!?©Ö½w"?z¹™Þ?íX¥	S)·?'Å­<ÇX/?¢_]Ç28?©/b¼_W¯?Š´Jkf?¤p"5i‡?îo>¿áàc?°G˜Œ¿›«?šb%ڝ)x? ‰"$%?¸Î¦Âê#^?º·*èШ=?ìø¤–ù?»­ÍqýI?«#—LÌÝ?˜§çe)z?ºÂ0Émê?«^ ‹?êõ€r&Ü?­±b+'à?'³FÏT^ú?m5oP˜e?­ôdáï?˜Vu{®×V?íåžVS?˜˜ÄépÊØOTHER4FGL J1620.9+4852?éòŽ¶š9@F>dÜY2À;'òvªHÀ<÷#ý5Je@4½ú¢É?ÿ‡ÝDUG?Ñ+ä<U?Ç#õ}›?ôý›yÙ
@·]`XZ_?ïÿþÞ÷¿í­x©_	{¿É£èg‡ù‰¿Þï0ês¿î
▸"?ØËWí»°UNASNone?íÓ­~JU0?´
õù OÇ?xC@¹±ü?w7€Õ¿mö?¯¼À¸"h?³ˆü¢l?Þ?ïtMlì¯?ˆÕ¸·I¶`?js·/Ë*{?má‡+œS?ŒO·0)ÿ³?"Zr0VÜq?í¼É®y?ŸŒZŒ€æ?	ÛL³G?*¥n†?¯ðîD_¹ ?ž]é"p²?ïƒO7B.?k Í¥šÅÈ?n=lÍ?Rä+qöwù?‡¯êtð›H?gÁâ˜ýñ•?ìu'7ò×ñ?¸°©aªî??' U}'?}lýÇ0Î?¹ÿcšP›?¸
¥—3]?î¤<5mþ"?¡yÆ"`=ˆ?vÅ2nþ¨?€‹8ðÞ?¢ã–Zþ[ï?ŸžVþБ9?ìf#M7k?§}]ÏJ?ˆKga¬ûô?…èj!€?¹Åx«Éƒ'?¦šÇ+£ù?îxo¢û8?Šc3>w"?8®9ê'–?qX¹š}?¤*ÚD먖?ˆËx¡Â×AGN4FGL J1621.0-2625?ÖÞ]C/@0sï¿@PÀ9ÆÕ©²ìÀ;t	§H®Å@»¿Nßáý@÷d[ËÙ?̈́Q2øzÑ?Ø"@Îé@‹6¿y@*ö'©¿ïê~ŸBP?ïÁ0αÿ¿éåϽ—ûŠ¿ç¸ˆû¼¤¿ï»Þ§j¾¿ïÿö$´ë/UNASNone?æœÀO(\?Â\4«¥­?"̈́† ¼?"F¹ =OP?хCÆ֜?ÁéÊB£-?ívoîzq‹?¯!­øØ6?¥œˆ2$P¨?¦aI(	€Õ?¢üxåX¯¦?™ö‰†<tÄ?ãéÍ¹Ë'?±ñªøਬ?¶x2ãvL?¡_ý=C\•?Ҏ鬒ѩ?°¼XžBCô?èUbaì?¢~Œ$ z2?²³œÿC†V?ŽgܱgÓ?Æ@ÝjÔµ$? Ý2kO=Ý?ޓ-F·­?Æ6Çî§Ï#?¬ñîî€hÖ?§ÑÍTҔ?ÝΔÝ"7?ƦpŠµ-Ò?éIˆNŒü?Â<=jf·?¾	ؾ?Ó?¼·â8ð?·©äÔü'K?¯|ãrë*?ÜöaQÐÔ?³kXÐ$í?Á£¢5cRú?¨ñ'q4µ9?Ú7͓¾…¯?²Ìš®Ã`?â$—R?°EXSòÿ?¿P lÝ?¢mCæŽÞ¸?Óô½º"ÂÉ?°ÔA>Çb–AGN4FGL J1621.4-4511¿å4kžxjd@
ª}>ïÿØÀ9ºÜ€žöÑÀ;n4Ïë@ï²>+3à@lX–š?Ô§]7¼?ÔïŠ|p>@O@4£v@+
y*¹<¿çtí²öaò?ïҀÖT5¿æÔÒ$ú¿â
Ÿû³j%¿ïÿyÈBúQ?î"ò¨ÿh+UNASNone?Ö–íSY?ÄWÜ­6ý?­ø‡«N…œ?¥¨,!¤ž
?ã,¯Mé?ÅSï§~p?àT\[¶T?Ê?-OÌúx?·-­ÚO?´¼j³@?ٕ¼ž#?Ç[ë‰â}Ÿ?Øa,Èi?²ÝúÓû}*?Â͗;àÊ?ªï¬>·c?Þ8/[ã*²?²ÈÆú°Ù?ÞïÈåY?±N8ƒÓTh?®h
·Mµ?Ç´Þ9HÛ?ÝCÝTÚLè?±^*×Q݄?͉:ÓÝډ?»Ó—™ü?³µˆ›¯h?¬(æ3˜ë?æ'7»á¡?Á$CtQ"%?ÐÊ)¤³\?ÆíôLS§?ƨ€@›ëG?ÄëÝ>	%?áðË
ý;!?ÉÀ‡NéG,?ËYüi
œ?ª¤Í%'?ÅLaWˆÒø?­cyE=N?ãÖv»‡Û?³ta"A+t?ÌeðZ»?®ÛM#ah'?³LÑ›IÑ? ­±«=˜Ø?æ|éÛ%€?²(j®'ѹMIXED4FGL J1621.9+6706?ßP×MÚ(€@C‡á2µ^òÀ;.÷<À<§]k"@;rW3C@§ÒŸt¤î?¿ìðXõ¿ºEik©q?ðÌgL?s³?÷,¨‡ª?ï͎É[ÿ¿êÙ"±ð*¿èÌÝÓ/g¿à‹ èBt¿ïüQ¿æ4}¿î¬é!í¸UNASNone?e{ž¡?­¸®èÎD£?dª;~	ˆþ?sñ}Ï?‰o—ºџ?¬£Af7É?îçàŒÐ»ø?œõaýä?ˆwŒ³¿ûý?YOýnUH?–È(/ìñ?'î.¨Ú¶?î7ž{;ñ¯?›ÑMfÅnÐ?Š|¨ùÝç?‰3XAW?¥æî9:?˜¬–'µ?î©$0áÊ5?†u,D/—?šq0žø6?ƒ
ð;?ZÚ?jIMe‰S?qÿÜ-bź?ïi,¶¹²?¬z…ý'5?"	ñè²}ã?šXË"q§µ?'Íás¼Å?¤Æ[dAØn?ìâÀêôޗ?µOëŠ.?¡ø›?¬ˆºÉÇ?¯Ûo¹­?§^Ì©'^b?ícßÖóIí?¢Á«Ëͼ?"md¨
_@?æ|!¾¶?°¨ &È? \ðÙ7?ë|LòYµ?§«]U4~§?·£Lg5?¦[€žêÊ
?¨ô§L/{?' HÉE6AGN4FGL J1622.0-5157c?çáë¾nT¿øÓíçÐÀ9mbÙéìÀ:´&Nyá@䉱ïý@ã¬BÊ?ąÿb$?Á	WC¡ë?ýö5{âÏn?ùDÔ:ªJí¿åvw@(d"?ïâÜ~E«0¿å`i,"A¿åFÁ+Xô¿ìÞJZƒÚ¿½Ãø<èÎUNASNone ?ˆ_À"êá?»D3zo¡'?©JÁr».K?¥	FG.Š#?牻øê#?¾×È º—?В@íì?ÁPùÍ`ñ\?µ˜pUè/?¬:(É )?åãÞÐõ?À½ÛÅZŠ?Éów™È@?®°Hà(%6?ºÍn±ÞV?¤ò+\có?æ)tI—½e?±åà5¥.?ÎepûžO?£T™?¿Ñä	ˆµ?˜z¸bD‰@?䁪#wµ?¦VKiŸ{½?ºîùÌ£öÙ?¬ø-«³?°¨eûú>?©ú²?+/?êjm?µ§–"yq?·
N>0Ð?²ÛEÒÆV©?ºrM'À?µÿˆf
?éÞGø"w4?¼shWî¡?¼µÕ0ëҙ?£yȟ¿Ä?¹ª^?¤¤KÛ={?é3ù™ßdª?¬fÔ^1P¿?¸™+÷F÷J?šZÈ'e3?ÄÞҚ?¥øNֈՀ?çæbÿú€?ªW CŸOTHER4FGL J1622.2-7202¿íÀ':+ŸìÀ/þKZÀ:}"ç¨ñ%À<|ɳ<ØÎ@¹âÖysß@$  0÷ð?ÂZŸÞ­?ÕðÖâz^@[è¡>©‰?ùzÛž?ïÿÝƒ(i¿ÝæüÅW8¿Ø¾\ý1§¿ä‡(mÀοì¾}ÖÅt¿ïÿ¤?åÉUNASNone?ۍ3«dX€?š®{—¿¿?Í÷Þ;'°Ð?¿zM'ɵ…?ÕvÝ6ÒO?Á´þfš5B?å§
NáÔ5?É ]
М?̥ҏÏ?ħ?zûZ?º¨Iäê>¼?·((–‹Âø?ÛHÓ2íh#?¶n¦ù>ö?ÕÅ«5ñ?´Ž"'ÞÞ?Íäz©\?¯èµ") Á?ãoì/¤Ä?£;ªÍ‰æ<?Ê@Ž¡ª? ÃŽi ¶?È$°¥'d?š)(;Š$?Ҋžêfe»?¿¹ýÌ#Ò?Ðvºm4òâ?ÁN÷ª?Üþ¦¨d§c?Ä;¬;æ=À?Ý&IÈBpà?Ì®}xÉ?؇؁`è£?Ì âÿû3¤?Ä£»nßv?¿¾È£Ùt·?ÔĶ
À'?¹,½8gS?Úxé$5-M?¹í ¥ù	¨?ÐÂ`γ"?²Ï;!u7é?Ց¸Ù>¹é?§ô_%0?ÔܑÐ;[?®Ã¦O‰?ՑµV…ë?¨kŵ|/CMIXED4FGL J1622.5-4726¿ê'mí™K?ùý ½é¨À9V3é;˜À:²xþŸ3@®hÌr3ú@tÝdʄô?Èë¨Z&½?Ïl¡ÿCÂx@Ê:#}?ÿx-
TQf?î˜ÓÁ2º½¿à´Ҟå¿ç€ÔÜeÇ¿è¡Ý4ùÝ¿éTô¹zàq¿ï¾á77¥UNASNone	?Ì^žëVêa?»*;ËƬ?ª}çTE?¢F®6Êò?ç@yÓ^??½ÍN×mI?ÐõéòÕÿ?Ä'.Ú«T$?·¹çñ*?­H­6è?äŽAOD?ěBì0?ÔJeø5?²·ÑMGÙ?¹ÖåæŠtI?¢iÀWis?âŸðGšÒ?³?ÁEùí?Á#%¥g>d?—yÄ''ÞG?¶Šeî?Ò>	ÈÓ?èåéóñvG?'ƒ-n
ª?ÀÑwÐàÇo?³,æÇW"}?ªÇ¼ÜXŸÃ?£tçtó?ê&>D(?¸0P¹D(?¶ 	Ìr?µ­oãö[¨?»‰úª«»?¶cpƲC™?麽	z
?ÀÃù.?ŧ?"ï]	?§‡Ø[^;?»Óƒ'"{ø?£…çƒXûÊ?ç¿ÆÿÙ??¯0å#n¹?¤H/µ…V?†NÐQúd?º
µÓ¿Ó?—›Óëé?ëyÆJQ²Ð?šöÔjø\ÎOTHER4FGL J1622.7-4934c?àZk›"€?·†×J)CñÀ7Ò'D:ÂÀ9bÙéëÂ@J2Œðø@‹$ÜX[?Á5šìð?Ô¥lÞ@9É oâ?üç`¬"{¿áø"0¤º?î[R¡ƒâ¿àZþ¾·`T¿è+Öþ)E¿îW}à€ˆÑ¿ïýÜÚa
UNASNone0?z*?Ýii?z6ؙˆ¡€?Ó öÍÌç?ÌÁæ·&Ý?åû0{%˜É?Ìä  kgO?š*M±c»?¡Vÿ»îul?ÛòUwÖ¦??ÃÐ7z냜?á6ñëÙò?Ã~bÕüæ	?´0pÄLñV?¤|ÐÞR™?Õ3 蜥×?µ8SàP-?âàasQJ9?¶5ÅdǬ‡?på!€õ³?VΌB3ù?ÉÊ`¨6j?¦tDöT/­?ékµiȊb?¦§¢ë®¸…?p,Á½Ø?hãÎ?ÔX2£Â?ɑ8ó¢µ³?峍{~% ?ɞøÖ7|?'¾*Ö>üÅ?Œ³(ñAÊ?ß´¹½rß?Çð(Ðy9?ßµTìҌæ?Ç©'šÏñ?¨Ú,_C,\?›•ò3þN?ÖuВ»?B?¹MËâê?ã7tðå'Y?¹§H·\€½?Q¯wF,?AF(C×´?ÐÖ#†œÜ?´!¥%ŵ¢?猁KÄú?´*%
îŸOTHER4FGL J1623.0-4624¿ïŠ˜çå¾@Fb\ìj!À9e3ÔBâÔÀ:àŒ]"Y@†zº±AV@ÛµûÏï—?Æë΅3±?®[!3‰ù?íºüÀ°^Ø?ù>&×/QQ?ïº8À»Çl¿ç*.<Sme¿êú©u°¿å>`"†É¿ç–&ÇUj¿à0«¼²UNASNone?ԀN6ê?ÄŠ&"?Öˆ =›Ä?B8z>^?å@~Ø©l?Ä=V'm®?Ûu5çmŒö?ÈàèçÏKq?¨"œÕoOò?¦e(µÂg?à¼?)>E?È`¥&••ÿ?ÚOïy¹Ä?µÀ õv˜?©ÒfÖØý"?š–Wúû¤Ë?á;M›5È[?´»Zwò_@?̅òœë?¡b¨­èîÝ?¦ÁŒ{½ ?ƒð_‰2…B?çrj²¼ˆ?¢8l»¼š€?ÅþÉ~䌇?º7ʔј?'';6@Y?‡áw',:}?éô;Èqã?»@ïx78?Å<ææ("r?ÀjéQ–²?°ÿòR¾ü?¶¥ô³h;?èÇüšd?Ãe2ƒNÃK?Êü\¥Á?®ÿD­ÔÆ?¨ÑS?#H³?•––@/Z?ç³èôºke?°r1ûĔÂ?±‹·…r-5?'‰ˆÜ0b¶?«ï"ّÞ?'QézÚ'?ì–ááåk?šbY
"ØfOTHER4FGL J1623.7-2315c¿»³ìT\@2"ëÄØíÀ9»øç
¶À;&ߢ'fŸ@_ºžLè@øb9°û¶?¯1†_Õþ¿XßÜÛO?´ýò^¬³¨?ÿG[iUŠ¿æˆ®Êä?ïüœh€òÚ¿ç%Ž?w4¿élëá:(¿è¢™ó[¬Ï¿Ú‰=UöØUNASNone8?íÐV©§P3?«nPÚ}?sp$À}­Ü?pƒ('36–?°FHe~ÇÍ?ªŽ8|5s?ï?8™¶º?"O²Dá0‡?y乃føÃ?€5ñ¿Ðƒô?'ŸÐä`F¥?ŒJE—Š9?æ|ÌÌþ©?°-}Tˆ?£RÏO›å?•Í(r°
?М
è j?¯kNÔ4±I?é+xåÖ?¤þm&ö™7?–#O÷Nb?xÍ7°5\l?ÈÖè9dЏ?£×æ ž£?ê8ò4=¨?¼«»š TÊ?"±…!&;?'aŠ'Ñ«?ę¡†øØ?»«¾ñS%'?íê­Z8'0?®bAk>Ä4?'xÜ,2°N?¡9Ñ®š?¨¼Fd4Õ?£i`†qt?â ù!"zK?²\ËOº¡~?°=¿é!‡³?Ÿ® Zៃ?Ö®Âs,?±@"_÷÷?âê$M¬?³¤ªÃŠ?¦¦N;æs?'¿Kg®ü2?Ø	b
GgÚ?³YëÑÿAGN4FGL J1623.9-6936?åä/]ÜÀ+í²'¸#ÈÀ:]½‹ç)À<uƒ/ÊÈç@i"¨ò?ÿãf³"@?Âçښ?ܺ?×€
Qh@~3Auì@F-ðS:?íþ'›ýø?ä:ÿ°Nè¿Ý¡ªÌô»¿ßBL`€É>¿î9ÎWçG¢¿ïÿÚ«² ÒUNASNone?æøEü0	*?ÁaÊq]?Ìê@c{2?ÀM@…1Ç?¬Òž³^ç—?¢ýêTÙ?씼SiÛ?¹êØ·¢Õ>?¯8ßÍ3
Ä?´[+ê|{ ?§{Zû_mŠ?¨@Ô!#?áMÅ,`f?·íÚ¹t€[?Öõ¨­L˜¤?¶¸Éfý\?¹»3ꊚE?¤´õèx?ëà"ÑøtŠ?•gA}"ØE?´§–¤2)?'=":X6:?¨§…"¤É@?'[Ò¬'G#?∶ËÈ1?Õù¦õw¼?ÕNï¾5Ó?Ãèqû½G–?¶ýåW°?¨íL®ñ?è-¾™z²E?Ç>)*	­˜?Õ;8?ÄY¿O?·g"Är¶+?µ8qÙ±ï?×út
L?¹2Íß¾¹[?à;Òå¦É"?»è—-®?¿ýèù~1?¨ã«h#?ç"ÁYÀ?ªD2Yӕ?ÅÃNx!éy?¨ƒµþ:iD?»i%¡_?—_žÈ˜æMIXED4FGL J1624.1-4941c?Ü1	¾º¿Ã½?æõÂåÀ9eôݍqÀ:ß`ݐi@¯ÈV"Õ@Û`
†Ñ?Ò:Ùâ)U?ä_Ä@Œ70@[®¤Ã™G@!­Ý|é?åÁ¡ŸØx¿ê"ɞoc¿Çnיå¿ã؀_5ð}¿ëæÕÂ>ÔQ¿à¯ÖòÀ|\UNASNone2FGL J1624.0-4941c0?¦ÞÞšW4?¤_BÄklo?°}æÌ•?ª,'ìŽF?ì~bbª?²Âd'ÐC>?·ø†ÿT?µN`Ãá­	?±ÏÏ{´Éy?ªŠ"n¡?êÆõNe¦?¸¤çÍ8•?ÊÌ.4yaô?°úúSÇ¡?Í_y4±?ªq7¤×ÇD?äiœ"ôé÷?³‰ÌA˜)?ºCb•ÌZŒ?–R|ª?·:R…Í£¦?–ÇÇç¹!?éÐI\Ñxi?¢ÉÐýŠº?™ê"Ëéê?'±XšN_?±T¤|̄S?©ÁX.Íæ?íÑÂn¿?­°†Ìå?£M÷­{?¤ùô‹ù5?±ZŠî ¨™?­†ëY9^?ìŸÖ÷·æ?²߄r[‹?¼©Vgý?¢´º"ÏX…?Ã=ˆÌ—È´?­ˆ_ê´?ç›z¯@Ó?±"5T¸£? ;'²ò<?"ÿ¼XùOé?·¥@ؘ? …•—ᛁ?ì7¥w?¢ãdÉi!OTHER4FGL J1624.1-4417?ÐCžã@
—Ne¾¡À:8;fÀ;EÝhüBÜ@äÀ^g@ä…BÊë?˲&˜Æ
?Ø/s?è£B@WÝ¢&e?÷s7µxó1?ïþsè¿ãã'ö»3¿ÛØ´¢¨ñ¿å‡ÐO¹¿íهÆ2~Ø¿ïùñ]¥Í…UNASNone?¾Uh|Á¿?³ÉÄÞۆé?£Çx´x–_?¤¨C%z«?êøÛeŽF¢?·Z•ï?ÑøØû™ü?Åó™Jt|?Ç£†c ¨?ÀK"‰xJ{?áÎaf;7?Ã÷Jò?Óu÷ÚRØ{?±B'Ò~]?¾>ÿžue?¢ÙNÃåûû?â}$ñÖ?²}¿3t0/?¿ê˜uéLq?"ÆŸØìŠ?Ë
˱ªî'? Jtl‰L7?å?úØÍ?¢Ti+ñ()?®jÌ*?¡ísq¢ë¹?­¹]üø?®¹X+ß-­?ì=Ͳi¸ð?²¼˜³Pàÿ?¸€ ˆe¨?¸º¯=ð¦?Љñ;Ó&?ÆÅç=Äå*?äªóQN"Ñ?ŝ…ñ_íë?ÅE]ç*µÐ?§¶žx€¹?¿QÊðK#Œ?¦µURf?æÄo(+î?°Î÷‡¿@?¡)ÿÞÁÂ?˜¡×=¯‡?Îêƒê¹Ou?¨ÌÃ÷ú?ç2¿<_W?¨óPö
àcOTHER4FGL J1624.9-4538¿â­8¡Î@®ò"z–À9½ï}Ѽ÷À;)²ì`@ub
fE@ܝ 6×?Ó¶@ï3?éDGÝå#@LRç-¡#@‹ä<€?ïñ©ûçl‹¿åø‰|ëä¿àø›ó-u¿îh—c^t*¿Þ}z¿ŽËµ¿ïÿí )k3UNASNone?Õƕ'³Wl?ÐAêc¿ ?À—îb'¤?»{›Æ‰U˜?àö¹ž'ó¡?Å×òV€?Ù=4@ï'?Í`Éñr•ì?Á<Ú·='?½O"êTŒ?Þ$Ç҉q¦?ÈKaé©ý?ÚNôUŽ
0?² 4Ž¡Ë?Ä}ž#ʓ?­¼G^,hæ?Ûr<˜Œ©F?²›;LŠ±Å?Äw²o–?ŸßhvZ&?ÅQ£ê3¸?§pQU?ôù?卪iT‹?©ôÔ‹?Èb¶°ß?¼"ºƒã¾›?Áž÷³;'?»0xmÏç4?卷"	"?ÅgPh›?Â}?à"~?ÄZ5^9Nß?ÌãÇdÄ?Ç=}%¼õa?äCn醅¯?ɤk5?ψ<ï‹?°_»ý´°¨?Çðy¯ïFt?²Zƒ5¹|?â>¿"v!?´äEMä?£¦<˜¡Fî?‰ÝfÈl2?ÉÝ 't—Š?´œWù?èN4¿n?´fN&ÚOTHER4FGL J1625.3-2338c¿®Ñ;\«"@1š'>[…bÀ9éÊ¥«ÔÀ;Î\ïÅ@
Ù æ@ê¬azŠ?×n†ÆX>…?ãb_p¨à@<÷S½@W?	*K-?ïÿwåëo¿å»Û¾,K
¿ç™ö!ãÕ¿ëõækÚC®¿ïÿÿÊPË?ïü!~|UNASNone1FGL J1623.5-2345c(?è)"\1•`?Å*i9nOƒ?¶ -´"™Î?·xdï݌Ò?ÄK_¶D™?¿tR¼;Ž?éêZå‡af?Æ#ë+³?¼ÁȳsƇ?ÁUo•†‡?³ë`ã:Æ?µb\¥<i?âße>¯Ns?³Pj
=ié?¼ÿ_54?¥Qs"ïÙæ?Ó]µ_?M?±Ñ™êf)™?Ö6»¼6Û?®ÄÍèÀC3?»½@°ÒÎÍ?™ŽÀ]äÈÓ?álú@È??°;3/GåI?ãÀð
w?…?Æ_°ÿ=/?Äs"Êe?Àƒõ¼ô×G?̈¬¹~]Ë?Ám'm
Íí?à@]~è¾?Ñ4¹»M•?ÕÌêHø[?нÁÆßM?ÃfyérlQ?½3~¶Ù	`?ÞI5þê?³"tú÷Ú!?ÃìǹΪ?ª€(©öe?Ø­åMk?²f¬Ã~*¹?¹à~Ÿ1"?ŸQUý9[?ÀüBæÚj?ª
R"úT?蠓60Ç&?®«‰èüÇMIXED4FGL J1626.0-4917c¿§Y¾{:翶aTâÀ8D*zýÍ À9Úqvdá+@<†¯Üüñ@)Á'°—?Ë;Á·šám?¢*	é¸ÀÑ?æÕÊ@qà@;†rJuD?áXsÉü7ô?¹¸"늿ê恗DU¿ç!Ú{9¿åŠ*@Ejm¿Üëû¼#‡DUNASNone3FGL J1626.2-4911<?¡¼ÝVâÙ·?˜ß˜´õÉ#?s}Äd ï?u¥òw¿Õ?î½6¢‡£?šê,þŸ?¿C§×lZi?¿ðü}êg?˜k¥)? q?™´9§Ÿ?ëT-۟<`?À/ñ¨VÿI?µ"™±7?¢\<)éÑ?°>jtÃu?¡<¦Od¶?ëX
=¢š?©ZÓo°r?Àõü͈?¤ÅŽîYŠA?…Ž)?q6â8Ȋ$?ëDj¹Ãká?¥é?™ÿã(?" ž'¢â7?‹ª>àîö?kŽ{,üá?jtö–Y§?ïKl'	
?ŽWèuÿô]?²º?%‹©?¯xµ4Ë?— Ãü»õ1?¡Œ4.Å`(?ìë±ûvi¥?²k{+Ö?°(}fý½?š®áWÝÝL?¯½TS§7‹?¡ÕÇÙY3?ëÿ
Ís?¦œAíÐ4?ªHbb~Wý?–7«4n%?Ejâ.ÛK?yÓGù[{?íÙN'ïÞö?™XvnYJOTHER4FGL J1626.5-4406?äZWÇàª@£&Æ=f"À97RÁmóùÀ:þ›H"@Eªs]@yä"rÁ?ÄÚ^ZÔ6ù?ű9ÉOj@
f H	"@¦+Š¥?ïÁkoº£?îÆ>¾+Ê3¿ä¸R÷ô˜Ä¿âçfá¶hÝ¿ëw¡Aƒ­õ¿Ý+m×sï¼UNASNone3FGL J1626.3-4406?æׅÕt?Ç ƒìfΟ?žr î\öm?™ÓÎöR:?ÐiÒ·Gp?Æ.Šµƒ¸?åÜc?•^eTÝA?¢cEˆ@?¡Íiʆçß?ÑúÖ;Uþ?ÀýS.r§?årÍÂã?³ûˆK"?©´­¢3Gà?œôØí]	G?Қ†Þ{\?²£3¹ï?äNìì@Ê9?¥Ú*CЃH?²t¾ª‰?'Î9{¥&?Òß÷Óê+?£Þƒ"qµs?àÛnUü"?Ä´<êä\X?°'zâ'¯?¦ÃpÜÛ?Ú)HjÊE«?ÄՁo^æ?Ûø,èÒx?Ê #|íø}?³˜"¦<"?·N¨E<?ßAm1'??ÉBDëcÞ?àøF†³I)?µÐ¶qñ¨Ý?°!ZcÓØè? "\ÈË;?ÚZdá'?µßÀú²?×dýŸl[7?­w8v¸í?Àä°pmÛ?¥Ãý§Rm?àU.‹.?®bâ\èËMIXED4FGL J1626.5+6257?ïÿÇ»•²@Dß°Õ À;j‡È¶½—À=
eÀN@ uVÞ^¼?ýƒ_0Ð?É W£Õݘ?°Bq>±—?æ¨B©È¼@}¿AI¿ïÿÈl뻥?ïü¸¹"Š¿ÊÅ¡ŠSÖl¿å
"Þ|L­¿ÂW$T9¿ãkŸ‹K"UNASNone?ï̈́¨ÏJ3?ƒîmÒ5I?:ÂÓnu
??	`¨³è?wo}Ãz–?ƒ'¬\ã|?ïåEÂ,	ô?jK¹ kZ?9ÔÀ(ø0œ?Ezà\ݔŽ?g¦—Ãî?f©m,—M?î茘)?"'ÀÐobœ?zîàŠ§2é?"ãDđP0?œ2´Ü`֔?'AÌu†aP?ïæàgfõ
?J;q×xÌ?<Ͳ©?)†øÒh™?e…âOdp?I,aaM?ï¸ó':½§?—L×ÛÞâ?NTK¿L?T¡°!Bc?»âïûÝP?€yÄ$*Ù?ïªÊK	¶?ƒZ¯´È#?Kx‹Y–"³?VßZ<?Û?ƒ•ä}Íq?õ¬0X?îDßmŽMá?™k¶õY?v¡&‰·8c?<-æÁ¸@?¨ÝäU¸?ã?—Á€ì¹!*?ï¿4¦Oàh?g8Má½T?K<í ¹©3?BH̬ËÙ?|þT!»u?f¦29sAGN4FGL J1626.6-4251?ïþq[Êy@>­\ÄüõÀ9«ã°> ÍÀ;
»y¾1ÿ@ÊÅ&@ù5žG~D?ÍpÔ©e«?ӝÁÓÊm@íÛ¢R¦?ö­3²_
W?ïõ=߉'æ¿äS«Èp¿ææq¹€¿®¿æì´ÿP­—¿îí47³K¿ïÿ¤''UNASNone?Ǎ½|fœ±?ÂþöâíB?©eٌnzì?°XG'™RÕ?è†3H¬u?ÃÝmŒ~?Չ
y Ž?Ĩûc'?ÅYx
Ы?ºú6±˜?ßÊ+ê‹ñÞ?Â&(º¨?Ø¿qÊȐ¨?³>už¢ö?Áo¼èöp'?¨Gá=£C?ވ¯À¼7?²¸
È^‹Î?Ç9ˆ_¾	C?Ÿ»4d"»›?È	Pv:? t[¥è0?ä/Iʁ÷o?¨u±ï8Î?»™:¹±›?²©ÞÆ?¬kê[ib?¦ˆc²!?êËQðìw?·'€¦ÈE?¾xkŸ ?¹ðGï5‹?Ю÷étè?Äöé$‹‰?ä&֗b?Äâ\Ì3ʳ?ÍÑ¥·è—·?¬ü{:ô´?Âq'òÒ	?ª¥£ÊÌ¢?ãïOH'•ï?²¨çªÉ—¹?®pÃõ7Ð?½•¢>.?Ëñ±¯KBÛ?ª"ßíÌ°?ç"‡íÛÌ?­m<‰í*ñOTHER4FGL J1627.7-5749¿ÕbùõN÷ÀȞºjÊyÀ:%µQàÀ;ï 8"«Ì@|T{,q"@‡ŽºB†?Ų`$'ì.?Ûk_ý–™@èAYB@‰,™»þH?ïJ¶Ýw>ü¿Ò^©Ã(ß¿å"áu¿èì]60¿¿ïýؾ°»¿î·Œ~~
GUNASNone?ØAà1ë?ÀŠöyՕ?Õ¢B G.y?Ämáî$¾Ú?ÒY|Çë€[?¼á¯ÔH?ԆÁŒõÞ?ÀðÞ-?ƹñF}%?¹,ÚûÝ?à"è×G?Ã/ë_ßä'?áÎcÀHD?³èºM ?Ê×¾d̀?­&Œøõ•[?Χ™AZp?¬'ô?ʞ´?Þ^õÑd?¢[ˆ©?Ò´Bx†¶?¡þW~?Ϸُl³Ì?¢EºÒ×ÜS?ÅDË-‡Å?³ùˆìž€?×ñÕ$µ"?Æ Òí¼ö?ݍu´%ü?ÃóMAHÂ?ÁÈoòù~©?»çI$â¥?ÐÄ»ð Ud?Ä@½Gk?ã+†zæ?ÇÈۆN
T?Ôè'°Œéø?±"¡¾ôJ?Óюñ}ŽÕ?µwG–:?×FI_gò?´E¬Më=?Åö­À[éú?›Ü,©:Ó9?Ýd'k§îÇ?¯ÔM€®•?× ´*<?­Ãc~•âIMIXED4FGL J1628.0-4920¿Íè¤ÿ¿Öù¦¸&øÀ9¸<ãÀ;^ݚzj)@b6¬j—?ú{à€Þ·±?ÐÎҀÀÚ¦?ê £ylS@2µÖ\?þÃ]¸Aû¿ïþY#¯?î÷Pß@—Ë?ÒO¥¤ê°¿ä}z´ÒD¿ì"{ýýFg¿ïüÂÉ=ÌUNASNone?–P'?"s'Áeæ?¢Z¹?œi×	;½ñ?î'Ð]ÈT?£Ë§èá¡?´
*^?´vtòuqÕ?Ír壐ñÞ?ÂڼކøF?æ#%Q¦ÄX?ÃYÊxÖøÂ?Ë>^Ô¦?«CnÅ©™¡?Å@üÛ?«ÕS2:?ãà^é*· ?±û 3ôp¢?Ljc—».P?©¿}GÃ&õ?Æ햂9?¬äz§0É?äby‰¦)?·ÀØJIôB?‰G/V"=8?‡€‰é}{?©ô8²µ/³?¥'@íž
#?íûŸ·Q À?¨¥†'O?£µ†LDX?ªhŸ>³¿Â?Ërt`=ò?ÇadPƒó?çè
ƒÁ?ÇÚÄ¥>›û?Áðô´ÈI/?¦º"üßX"?ë±I8®?°8èœx?æ˜Ö€Â-?²ÆѺ+ç?ºØ5ò¼[Í?¤²?yYá‡?ÆÔÙò¶R?·Ú—´PÏÝ?ç"
¢V"?¾§¹O¶OTHER4FGL J1628.6-4553¿ÖG_}lj ?ÿ<û¹IbJÀ9DçW'Ž
À:ÔL÷)—©@L;´4ç@]X…Ó8?ÊðΉ»U+?Ë0¼
‡ÃX@2/ãšj@÷jt6?ïëÖï썿ä­úNw\¿åé¬Áêp¢¿åË»Š…) ¿îۚû™hò?¿›šOÌñáUNASNone3FGL J1628.4-4546?ÃH;®?¶Ác̈́ؗ?¢ü'šéó?šâFimmF?ê
å¶ð?¹Ø›D(?Û±£^œöú?ȬtV'Ý?°Z¼ÍÆßÝ?§#‹yµ‰?àÖ¶Á®È?ÇRVvÄ?×46ÿ×¢O?´¨YÖÚš?·NõŸh‹f?£ ¸™Ow?á|Ì Œ?´ªéðÑ?ÑV^Ë+Q?¤ê'΁áJ?¬Çñ"‡Ñ«?…±Ýˆ0æ}?å­Õ·ñ¸-?¦Ji6£¡?¹]wo"9?°Y8쵿M?£¸ø÷¦?™!r_{¸?ë£àæ›f4?³¿@9"o·?ÆÞݵA.¸?Á1co'z?¶}<ívY†?´™Cn7í·?çx õf?Ãêè^×.ƒ?È꺧
þú?«Ö¶óu?¸,lìþ¡?¢©?Ô×2V?æċÈu¥?°ªì" B?·PúÌíâ?—èóI
e?°êòÑ¿?"™V`†hê?ë׆—¼Ó? Kf…ÅýOTHER4FGL J1629.3-4822c¿ì*Ȳ®5?ÃÅR.¸ÐÀ8H00IsçÀ9¸ÒãgC@¼HOúê@zÓOž?ÉK⁔ë	?Û	읢'½@Dh¢€Èè@ÞN«´¤7¿Ì°¿%j?îÏ27Š°É¿æ€‡yÜdð¿ëõUҚl¿îpñÚ£O¿ë8¾"UNASNone8?œÚh¼Ž?ž	š€Ãa?¨¤W;9â±?´2Ì$Â?íŽçFu°0?·CàØÜöG?¨¿ò*Ì©´?¬v.ǝö¼?ÉùS_ðÍÕ?»=¿Ç3cb?çõ¬›º?¼ñî"q?¹IèYÚ·¨?¦ U¾
9?Áº~ãØ$?©¼¤7a©?è'ÔTð6"?°îwµñÁ?F£†
#M?tø~(¿YÏ?Àµ=0"z?QjßOŽç?ë{"ÈE÷?ŸšÓ<cÅ?‰ð2Iפ?Š6dž˜º?¶¢Þъ‹?»N¦½TÅæ?ìÃü›5iÞ?¼Vã
?—i$(JÄA?¡F"XE»?Ïa°Ÿ¶5?ÄLsQ—ˆ"?çlJ¶²"!?Ä{I['v?°µ@"‡Æd?žAÂ¥,?À ‹ÓTȧ?ªˆ&¤‹cl?éá4ø§"z?°cF#å]H?p²]ñ.ú<?]¼£Ë}í™?ÄgXœ×Å,?ªcð˜s?êÄÅæPé?ª¸?ºêœøOTHER4FGL J1630.1-1049?ÌÃäç1@8Ô³_=}9À:™Xù–YÀ<ÈÑÚRÇM@Í_íüG@ÖÝâžÆ)?̳üqU-?ïýò߆õ@ü¥zxl"?þƒÞ©Ä	/¿èQ)/»¯¿ãý›6QË¥?´Gz=ó>¿âWŸ¤¯¿ïÿÌhù¾¿Ú•©Àª€UNASNone3FGL J1630.2-1052?°Çäž!T?²çH+Xl?íFjtµV?µø¸êÀô?"ï!?'ø
_'v`?¥3õù1}Ó?¨"ÿrdÂ?í'\Ϲ?°öfá'?¨V=Hñ¥?£'ª²³«?Ç".(1wq?­Ô
8/u?æ"uŒ/^ù?²ìbó5|?½÷RmœL?¦*ùˆ) 1?½P1[‰"?¡2ê æA¢?ê §ø$?¨~£½íˆo?±ïôöÁÑ?œÙc÷àŽ?°T@PìÆ?³VŠtÒS¹?ìÞókzªõ?¸Áé† R÷?¡hŠÄCÛ/?£¹RÇx$)?"'f}2?¡"ëWöc?îæì?­'¿mÑ?¥¦{ò{2?£›b^©_‰?¾3'(·b?¦V÷Õ¡ù?èÌ(Ë¾ý?±òzq»M?»k)Èëµ?¦Ì´LnÐ?—©èÁO?‡‹$b•3t?íçZ0'Ý?¤.@|"G˜?±~€2.?G?¡ŽƒÖ'»ÙPSR4FGL J1630.1-3546?ê.¿Kz°@!Zt֐›À:o¶Ò"mÀ;Ҋ,l@ .á¿Î@´"¡ºÐK?Ñ¥_ .^?Ø`etÎß@ÿïÕ@Óo¦©?ïýœ
`{¿Þu]¿ä'"Ð=1¿æÐ6y8Ñ¿ïÿÿ)@k*?îÍ<(¥:¸UNASNone	?æ<τ?É?ÁS·lé7g?°Àç÷ªÿ?¬®cšÎØ?ίPÅÀ>?¾‡Ð·p¢³?åôòC1‹œ?Ŕz¶%'?±:0¦±?¯pŽÉ·ª?Ï£Ú
'Ã?ÿe®›?ä¢Å5îhB?±Ý`é…ÝS?»<ܪ:{§?£Ú˜äÔ0?ÏÖ|Ó)!%?®$Øáð¸?æ¶BþhŒm?§‰j
?·4ú6ZÆ?•5Ñ[vì?Ɍvþ0"j?¢Y>êßLû?à·èg·?Ä×K©ª;†?À_¸4ÂÝé?ºUˆ»W7?Öað½Þ?ËU,Æ÷:?×V¶£ž3?ÌVÂïÔ8Ò?Æjtñw.¾?¸Ƞ¤p?ݱnРÊn?Ë,‡¹XŒð?ݳ	çäg?´.q5E¶?ÄÞªÙ®Ò?¬†ã[õî0?×Ý¡{D0?³HڋŸ1?ÖhE]F?®½Ã•L ?ÈO¦é/ÑK?­àÿšæ‡?Ýoç.!üT?°}rT)ÊMIXED4FGL J1631.7-4826c¿îçn¯hÁh¿ÇYϪ!Ò
À8ª/?ˆ¬À9ö¨y0m†@ )±`_¼(@$,!Æú%?ÒÂI;2[?ț:)Âq@Øm.׃à?ö­Œj1!?âÏàèãƒÈ¿áb×ÖK¿ç…¡êöÙ¿æ/¬*•ÕÀ¿ë¬] l‡¿Þ&«»Z3¨UNASNone3FGL J1632.4-4820$?Ÿ©´|›rg?šÜèæÃIê?–#µ\…Ìd?˜7ðhO£?îQ"±
ºº?¤¥­™ÃÅn?¦—±nÝA?±Ä­üI‰ƒ?¬Í]íü/V?ªwê©Hè?ìɯ
w?¶zۛ?[?¸ŒÉP¼<#?¤«rzÍ?¿^ºö`™ô?¨Á±ê?éwè]?¯xû¡Bý£?—"£Ö3?p§•ÅùmÅ?¢Ëxïíó•?†×2ÓÓ+?î\ê`Ó̾?‰T·½F?i$_²?‡ŸïZQ–\?ö8)\Þ?‹w_‡úà±?ïc¿ß?•8X2²_?—Ð/¨›1x?¡Y*ðlÛ?¯µ\{})?²fÏÆHÇ?íF(»,ˆÁ?´l[±?³zçh3¹ú?œÓŒ{ñ4ƒ?¿Ò6"; ?©ËTç2àš?é–\@{MÝ?­‹jt!?l•Ä™=Ña?XuŽÆ?¡ã"0g+&?†Ž3Ï?îÅ1øBì?ކGR0OTHER4FGL J1631.7-2319c¿ïÆËŪˆ@0²Ž´cI{À9éŽuy)À;_ŸÐê@ͦ;2±@"î¿eÛý?ՔžÝü ?çSfåg1@
ÈÕ[ç‡c?ÿ"˜‹Q­G?ïõûg¿,¿á¿Ú@RÖg¿ë{τ7¿é¡P°¼¿äV 7˜s¿ïõr¾
—BUNASNone2FGL J1632.6-2328c ?ãAKÚýoµ?Ç"¯'—¨?§b5»^÷m?¢P^'­·ì?֑!'™A§?ƸÑFâî?ævQ7w‡î?̶DÜ97•?ÇnÚ^íû?ÆҊžK|x?½oÁŒ…g'?½M2DÃò?ã;0"Ks?²©O>ùÝ?¼'•Üu·<?¦!ÚÍß4?Òi4(ûK?°»Ø©Ôï?Õ|txU…?¨y¡NP¨?ȵº±4â?©uË}$?'?Þ ¦3
?¬Ð®3?Þÿª¨":8?Ç?Ôû´/·?´—sW±.ñ?¯ ¸pð8?ÛÚx›öì?ÇáEÊål?ØÏrmt'f?Ñ>MEá"8?Ü!csS?ѯö¨=vX?ÆT@–j‡?ÁXãÞ?à'ªn܊8?²8a
&¨7?NJÇÞjH?¬fÃg(L?Õìå¾W¶m?±Àc
³?º+''"ãÁ?ž|"z0?Ðø®ˆÐ.è?¸—õâg5;?ä>6isŒ?·á±
{)MIXED4FGL J1631.8+4144¿ïÿÿD¡Î$@EÛLÂPrÀ;zWûi˜JÀ<êîê3@!xáî'Ô?ûg?>Ú0c?Ð$a1s@?µO%,4fd?èË.Ò{bw@PHµP"R?ïö]¿Î¸¿éµyÿ ^°¿çëWÒNí?±·K†;B÷¿åreÊÞ¿¡°lnéÚUNASNone?á /º?Å!CéÜ?PN—dÂh?x.wh•‹Z?§#4Ä#?ĵQÓSÆô?况:š?1Õiñ6Â?V´pÈJ?[—©ë>±?'½;Ä®¢?~~fL
%»?î\M5'Þê?›"1K©+?'Fº™Kú?‹{-)'?¥©~!ŬÛ?˜,ñË=?ï†ýžÑ½?q%ëäúr?\Æ9÷¦ÌÔ?GBþ%õ˜'?ŠãyS×W:?pªè+7
K?îÄöÑü·?¶@ðIaor?I¼Ž3øÙø?iÍ?£I¥¬Ë›7?µÏÌ@~Øö?ï:5ùa*g?"~a	&î?`L¯Ïôœ
?hÅóÍÁ6:?–¯ªà»WŠ?"MK3ñNU?í´W֟D?Ÿé?ªŸ?sŽùñˆÄæ?€3p;òŠz?±$QëÞt?Ÿg0÷³o?îCÝ붥w?'êGl
?uÌlÚ
Çþ?jJ`äUÜT?©"¦ª=?'ægÂJ׃AGN4FGL J1632.5+3839?Þ%¢ô}@Es£]gº#À;k¯{ƒ.À<™·•-#O@–A€h@EbÅÇõÍ?Õò£@ao?ã÷&<ª«:@jÉ¢uá.?ÿÇyü›F˜?ÞýÑÒ¿ê.!EÊål?»!Œ}ãkÜ¿á‰Õx¿ïÿøsCÄ{?ï¢,_Ú[+UNASNone3FGL J1632.8+3838?îs
dË?¨_5­nØ?¢&ö¤až«?¡ãÇM¡?š#®ìù#S?›ŠÁa/?ë#(_Uâ?Àsd%Ä`?·ROßw…"?º`¼ÿá]d?¯(ÚOþVC?§.]S Ä?êƌ›¦±}?«ŠÂÖȱÝ?³º¤£Y©?¤BùŽq©?¶ö}ûLu?¡†û'e«?éÐl¿ú_
?¢Ý™dõµë?·©=ß0=?›'K³Øk?¹Ó\!ر¡?—žw\ªfK?ëj'âû–?¶éŽ–F®?°'ï3o'6?©ÀÐ4Çn?´g‹ÀÃ?³wb?㊰ö,—Ž?˜àÁ q:?Ï}ã÷?Ê"»ž§ ?ÂW¼CV…·?µ_üsfP­?èÇÎ
dˆ?²*?A$Å?¹{bü€lî?©ñП6³é?Â÷/G§o¬?¨òZ›š	]?á‡ýù¦°À?²»Fd(Ο?Æz»¶M?°é'¤ÉHj?Ѳ¦ŒWwò?°2cAGN4FGL J1634.0-4742c¿ëlÂ8²Æ? ?áÜ\WÀ85O«8þNÀ9Õt1*Dw@y(

@Ývh<)|?Æ7d+xª?äÃf,Z@f×})÷J@Œ—Å¡_¿ì.
Ää ÿ¿ËD€7Ñ¿ÖÁ'¡…vL¿çëx‰~™c¿íÍsñidH¿ïÿXÛch…UNASNone2FGL J1634.4-4743c4?‹Ë'î'_ã?UWH±â ?Ýu^3ð{?ÍBï•ñæ¯?àÖ"ž»l}?Í+5W§?•²'v£{?ŸÖ™ª5ž?Ó(Å­/	?Â	TGTþ4?åÑ׉Fî¯?Â"µ—Qð?°~¼ 9-å?¢ã½´hîO?ÙáY¡±ëö?¶o[ø¤A?àÿ{›VÞ?¶QÐ00SÃ?ux´Ý;?]05d×>B?Á¡˜e*ëÖ?¢†i˜ÎW6?ël¨ËChh?¢ÜQMp8\?zX³±5S?ruùx˽?ßc2v ™?ʙª‡8Õ?à¶Á-îa?ʀˆúB¯[?'žÒ‹ü·?‹ÊAÈ?׬œº®?ȗ/¼± Ê?ä4®v(-ú?Ȁa&¥?¥-GÏ·Ë?˜¥¶XM;K?ÛP).ˆºµ?»::ʒq?áë²s¹?ºª"@ŸŠþ?R®hm-©&?A?Ôæ
?î?Ç®ÉÛÅ|æ?±Î™3¸×1?ê
öTÊK'?±ØSºMvOTHER4FGL J1634.6-4324?éõ[¯±¼"@ýñ.ð®À9ã'Æf>À;,èI*}@ zËA1xž@ A`ó_ß?ÄkÝþ"…¿"«¦Â?ԕcߣi&@ØÐ,}·f?ïûvΓvj¿ÊQ§g'à¿ãÌxéö©¿âÊÆͯJÜ¿é(€‡yÜe?¾¤nò	UNASNone?á&ò´K?Ä	_­Ã$á?}õçŸÍ?'?tÙDÒ?ÝKÚ|–\+?Ä)¢ÌÚJ?å؍ãWþš?Ħó‡ª6}?‹8
(*Ã,?rÒ ðQÁ?Óu#ÏNB"?Ä­øvHÝ?åÂ迾ê?±¾JVz?—j£þE—n?‹ÛHªW›·?ÓMÏî·¥–?±PcÚ?Þ?è¤PÏÖ?¢ô7~8
?'hœvð®ž?d¯‡Š×î—?ÎzäôG a?¢‹¸&éV?͐hê
†}?½Ö{õ¼'?"m‰>í!?ŒxÜW%Î?è}
+¨?¾á¡Œ÷¹?܈.ev¯è?È'"²÷'ƒ?Ø"+Ga?—+0,W?áD†Ž"Åß?ÇÊʍœ$'?Ö¼É=ºå^?³å¼+·µ?¦RbmEnB?•X&¯,­ý?ã<u:®k}?³òû¼	Â2?Þ®JQnò?°ÂvAŠ@?'‡†2
ã%?~Ÿí\.Æ?àž¥?°m²_¡ÞMIXED4FGL J1635.3-4159¿ÇÊç移é@
Ϙf"²ÐÀ9Ç DC%ïÀ:þìÁ^ځ@´°z[»¾@‰'¥R5?Õ˲[‹à?êùÄ¢0ìÝ@¸à†½õ?í(iå20?ïþ2Àœ'È¿ÚFUú³dò¿ì†úÆ[¯¿åÄd]øƒµ¿ïþÒn¥Ð?ŒÑt§FÖSUNASNone?Ã>"ye¶W?Ç4î';??æ5žÈW?˺—/çú?æFÑyô|ƒ?Ðå‡9«Ùs?̨>ÚӘ?Êv&Å3Ú?ÖF¿åÆ÷?ͤÍ6Kê?Ûe!°m?Æöø±?Ø©Y.‰D&?³–TTÓÝ[?Æ	×ôbë?¬µî sJ?ÜQºØXœ#?´Sk:ã5,? wHy†??aÇãyé?ß×S䝾?´²~l'?ÞÃ맮Z?³•Oï!N?Æã5JuÖ,?Éä"÷jÒ~?ÌY–¬ Ò*?Ìk¹a‹
`?ã0ÍãÆJ?ÐÛ¤j»?±Î}q²Ú9?»'DS?ÝÓP_
õ?Ðhä݇&?ݹDJþ?Í=QœLHÐ?ÑDL=ÎË?±0ü "y?Ê!fÍ>Œ®?°øÓú‰5®?àé&'uo?¶¼…5lE?uÌ¢B{Ú?c5Šjðke?âhŠuN<?¾0ÜE)™›?Ú׸Œ²`?¾Ó¥ëÕMIXED4FGL J1635.3+4258?¸ ~—ãö…@E;Ÿ<pÊÀ;VzKöx˜À=WÃ5tV@©Iu¿Ê±?ý1ʘ?&†?Ñ:"Yd?Þ²¾äV×'@©äðl@
¨ˆ±>üÀ?ï 1-Ÿu|¿Ðl¸þæ¿Ô[ÉàhÚ¿ÞaŽºú½¿ïÿÒ³–šâ?ɀ:MèUNASNone3FGL J1635.3+4257?ïÆGâ#?sb³:ç9?n1ö¼Ç0€?h÷²-÷?kËÂboô ?d«"ܺ‡Ñ?ïiK%BYÂ?Œà
¸!?sL‹šº˜M?wôÁÐõÇ\?ŒðÚÕt?"±iìn,ø?í¼¨0¤ý??Ÿ™òòàº?¡Àɋ;º?–£¡€#îö?¢t³iÑ	Z?""ÿ –\?ïrH
Êx#?l'" í4œ?€e2I'`?a°€¸
–²?ƒË:—??bReâÏ?ïv$ŠS?‰å
M??ƒ˜K…ÎWZ?€P6v!+?}½#Ñ/Kâ?y>§ÕLpB?îVÈÕ
M?ª¬€‰Ï¸j?‰$Èyex?—¹Û¨?¤^*=ýLÙ?£]ÀÕaM?ìY3\½†?¦¢Øòï]?¬Öᵨs? 	·eT?­•è‡ƒæ?š³°%ŠÁ?îvŒM˜î?‰qœäøs·?'ŒÈ(aî¿?}†+ÙÍî?ž¡¥ï¢ÁŠ?'\áæ"£AGN4FGL J1635.4-3249¿æ"zB]¿ñ@#±vû	 À9ç$Ã-èÀ;²F;…è@+hÌÅ@è¡ß¹8›?²¸yƒ¤?Îɹ‡uª§@§æ;2Ûõ@ür׸ä?ïÿÆ>"8¬?±é""xi¿åHpSO2¿æބ 
Q!¿éMd6á=¿ïüNÀ,€gUNASNone?Ý3ÊÝ´Q?ÌÙòéÛÀ?¡k¯47I€?œÀñ¼	J?àc«'$uð?Ìót ¹3?æCYb6?ÄSR'Ok?¾LÚ¬¼êŠ?³ƒZtâøU?ÇÌ.L²S?ÀՌªÙï?æ˜8ovõ?®CV¼±=þ?³Á¡B*? Q­]ú:?˾»xwÇ?©¦€d—ÃÑ?ãz{kÜ ?Ÿ'úa°t?Â-ŒL¡e¸?—KÓ¬Ô¤?Ïè†î)Ç?˜}¹V\ßÓ?Ôö||?ÂJ«k‡?³4`["¹?­–e‰$?㓞3m{ë?ÄfX—¤T'?Ú¹™–â?Êv2ìçI{?ѸpœÂ?Æ0ò%ÌÃ=?ӎÓxɦŽ?ǁ¨zpE?ß:>N^ ¶?²Î}qJ&?ÄEc+É\€?¬.®8Y…?Ö£½1
?°ÕH±Ê'á?Ӏd~Ú¦?¡ð³º_Àc?Ñ´fW*'?©t¸˜ö!(?Ûoç»N0?¥ÖUZÒðMIXED4FGL J1636.9-4710c¿ÓTÁðyÙ? š&	ÔëÀ7˜ÜïY¿À9IeVÏ@6ë¤~O@‹jËG?ÀƇ8n—?ϵãfÂ+ß@qIáËa"@áIÈ î?Ñ~Ç[HÐÿ¿ÙÏUàW¿ßgçšÙ_­¿éb—oîM¿îàWÄ4?§i™v´UNASNone3FGL J1636.2-4709c4?'â|{?€?]X@;?±×$[ØW•?²wÖý'Þ?í4ü`…ž1?´Sw*Á»?ž1kR<r?¦oš.ÏR6?ƉÉ?ØÕ?»ÇÅxX?élWÑ«·?½âQÄBæ?±÷¼2ZL? ÌY›ö´?Ém¦E¤z?­¶àÌ9þ?çeÙ>±QØ?°Î¸¶‡"s?rÐ[¡‹0m?\¥-à?­Ð"øø?Œ†+jÌY?íýV™-?o"àp;Ô?~¶OÙñ?wšÙ´ã‰>?¼ÞÍf‹á?½'îø¤I©?ìCë;Å?¾\§†þH?þ÷—P¿
? J̓'?È½ÈÍä¥?À"ÀÚ®ÀP?é"Ô¯*‹«?Àæ*²ÂEÆ?¦ÀúõhÈ"?–'ŒÆ2ºù?˸'»m˜¤?°ôo¯v‹ß?ç¥ËáÀNå?±ù­©¼"€?P$V¨V–}?@"'Ž°SÄ?³}ºì<¹ ?›BÎgÉÁ>?íˆ6wWǵ?›hÛôx†{OTHER4FGL J1637.3-6325?¸ÎöîØgÀ%«ËÉdcÀ:¦°ÞY½À<!<(F@ý'_d@@@¡°¿P?ÒJ¢e›?Òò=ºË˜@ëó{??û0¬%~é¿ìîX}šŠ…?ï°*À¿ãOøØ¿â†ðY|s¿ïÿ']<9¿ïÀöÕ´ÒÛUNASNone?ê ³Z_ó?·ÁosƒÄì?{v`2ƒ?ˆ=Mƒå?Ãp*h?¶b"›0?ê"îFšE?ÁÝResú?›ëx°û<?»¢"%L§?ÂnäøpGC?ÀK/3'?ë%Ó!-TÕ?¦MA×YÑT?£ïyþ|Oå?"!j?If?¼Ù©÷W1b?£8ˆÊ?ê½ ~²"ï?–9 Y¨*?¬¶x8ìs?‡Mȼ›?»·»O™<Ê?'/©ïZÉÙ?ä¶ò'Pœr?ś™ÛÖ!'?Ÿ±/Ë:Iª?—õ´§°ìC?ԗݳ¾£?ė:ÕÐâ?å£8dyã?ˬ-ŽN›?¯Á×jÿ`?³,àâ?ÐÁU	ò?ÊcÛð^Õ×?æ™ÂIn¼?²æRv?²èÛÍÐì?…b™Á÷K?̖kK?¯ÉY—úFÓ?æRZ\m®?¨ïŸT}?¶EЌew«?Få§+?˓­|$"³?¥³uª$vðAGN4FGL J1637.5+3005?ï%¥šÈˆ@Dd| À:ãi:V=#À<‡CrE˜@ùrŸ.ÙÝ@~³¾"æ?ÆÕKÚt?ˆ ×üUÑn?¿Øš Õ£
@ÈYÖ5+[?ïü—`uÖ¿èNƱ¿åo—Òïü}¿è‰/žÔ¿ïö(°ù1°¿ßÚ{v˜ã'UNASNone?ï-å‰Ny?µ‰"O:5?–,ä³ 
_?´Ò›÷J'c?pY¨ÆeÞ	?‹}˚¹"x?ïxñÒQa?ŠHZ.A(a?mڣѶ(Œ?r9¿"=Q?ŠLâpråÃ?…5ëÛl"?îø9òž?µ¤=´?}ôl)]Ì?}Ÿ'¦]ÙA?™{ÁjiÃ?ˆ®¶â)Ö?ï{Y\_ê?o]‰í­*?€5ÌwµÁµ?fF±ò®AG?€ó܁ã®?`y¸"ìn?ïc–wü?¨¯&¹,ð?Š-Z9<?§Éyç9Äú?yÚ¡ÚB?Ûӛ3$Ø?î'9ÅæÑ?¢¬{P?ðð×¼¿Œ?†7vvÅR\?¢îE•ÑÝ?ž±ñ?¢÷?î.šVFÍ^?–÷äèk?†?ì3'Sü?'Y=鄐`?§†_Œà*?"¿¬T'¥?îf¡]–?Ž+²¡­ƒ>?˜ýwX‰Ön?†'§±/œ?š.f}ŠÖ?€t}¼×~ÝAGN4FGL J1638.1-4641c?Æò}ûZC?Ê¢œâú5¼À9·ÛàfÅÀ;`®­ýÔ­@ §è½@G'Ñ(| ?Ö©Q2!»<?ïÕÿ™'Ú@ò¶ä-;¢@&½cÎ0¥¿ïõ~̹­?ì!S6Þ¹^¿wõÚã¿äúf¼Í{¿êï…>BÛÈ¿ïÿåþÌúUNASNone8?©×Éúç:­? Ÿ†ùÔ|?£uÙ¦é?›½ÔÑù¾?í+%ÅâLç?¨ÿÓ€'b?¥k`;Î ?®g+QJG?Ïj¯:."Ö?''èŸ?æΞ-Ò÷?ÂâzÍÒ?ÒÛD2Σ+?°î§k}ø4?Äßl›£xÚ?­':ê¢?áZ'¿¯Ð4?´›º\çõ?Çç£Erƒ‰?¤¢¡Ý¹BÒ?ؕa,&	æ?²«É(Ó?ÛvÍ1 ´V?±'_ùtQŠ?•UˆŸU®#?Ž"£AXÒä?°–绍¾?¨¼ƒžB'C?íBvüéç?¬ƒ·gÝJN?šP*å±Ë?£JV'N¨?ÔÙùƀ˜?Ëd%âpU±?äÀÅ'pÛ?Ëzž›zß?ÃGMÇ^#?¨Æ¢_g£æ?Æì^¼½¤Õ?°™sSë­?å}}^¿B?³xñÕÜ<?°&ÝýÊç?™QҖÌpî?Ü֒Ÿ$?» @Tµ?ßÆhsu²?ºg¶"ôfOTHER4FGL J1639.0-2727?çÍgÚãC@)"¨ŸÆÚEÀ9ÜZ°O¾"À;¹¶à…@Y¤¼e@컚ua¬?ÃWq–ë?Áûÿ)ì7¡?üÖ$ê›í?ý['l×CÉ?ÏòpËD7¿â:7žÒ¾~¿æµŒt)¿á›>¤€¿ë¬`Eºõ¿ïÿÿ>¹úUNASNone?è=¹Y'Ž?¾LÔÄèÒ½?"ìýì?ÞÜ?Š¸–Ìð?ÌkzÞ~·&?¾&wߛ¥?ìV—\Úe?µü'Ex¶ô?¢3¬¸Òƒ?›6YkFÄ?´1qj"?³¹?ê'N ?ªO—Õº«9?§Êw"š`?˜6à‰9œ{?ÁÕp'ì?¦møcÐö,?élÇþÔ(X?—PÜW:?«å½ãa?'±–0õ"…?ÃSšÖIg?"ò¼f?â­¿J°?ăxׇ?­Òo aY?¢ë¼RzK?Öê@½¬Àµ?ðêâ:R?ç4ª+¸?ÅÏ6g"×?¹'dÝÀ?·@ð
®9?Çúç½>?Á:QA—¿?åÙSì™ÏR?²yˆÆÒP´?µªÏa|œ´?¤:©ÅÇÜ?ÍÅHœÚt^?¯#£§ ª?âk–Ùö«î?¥zz
+SË?½[WՏÈ?—wæ±6?ÓÑüŠ]D1?¤ß‰aöjAGN4FGL J1639.2-5638¿èrÜ×˝À+äøé‹À9ñ¿ä†ý¶À;¥0°¡óÛ@sYùñs@ÝڋÒ0º?Ê÷8[;:?áÉø;æ`@:k
•ù@n‡/×?ïޝåX´Í¿ÝYßð@¿éÕá"oA¿ïýð@o\¿æ)f–7Š¿ê°ßьO.UNASNone?çëÌ£'å?ÁŸã
ß?¨éÎ[?£‡Èg]¨?ÊYí ñ–?¿ô½ä¸¸?Ü;ü3ê=?Éòï_.?¾|ù{?»ôPInˆõ?Ü#¼Èd?ƶ«Å‹?äªuç㩈?±‡RœQ|A?½!X?\6b?¥äVG³"ƒ?ÎÅ|@Ã>¯?­[ßP'Q—?Úm!í]?¦ˆùŠÜA©?ÏÀBõ6è
?¨\>óšfÕ?ÖqqBžœ?¤/8Zm"?ábó%>?ƄEev³?²|Y^¬bé?­Y…ª¿ÕÅ?Ø&#ÂÊ6è?Å36tlt¯?È2õJÅK?Å0Ý9ùÃ?Ìt
'±÷<?Ç)†îéy£?âáðž@ÐÞ?ÉÀ>ã¯V3?ÜdŠŽcÛr?³"üôc½à?ÅËj®ìß^?­4¢*)!Ì?صÀ%´ß?³0kñíM?¾6–óœ¡?œ5hÐJœ?ÙI
uZ ?·™UØÍק?ß)M>ª¾8?´{â	!MIXED4FGL J1639.2-0946?à¡% ˜H@7¡Â # –À:òþUÀ<åê«%@ òæ0v@°nºÈ¾J?ăùdo¿¦|c /Ø,?åKÕ@Ž»o?ߕ<¯« L¿ïí	î–K0?ïP3ôú€¿·Ux­eÔE¿ë¨F`®_¿án•Š¯œ?ÔÉÞZ鰈UNASNone?ïS¡ŒÏ~$?¬"MT>,?ul£ÎC?ªêՎ'Ñ?GHÅ¿Ýé?'"Ê"Ð?í¨W‹ñÕ	?µX"9à?•"y0te?ª["~Á^×?¦¯Åº<?ªÏGñL ?íÈ6^¥–—?žèŽ¦ØË?"n:¬_€)?'|–{}"?©E|½¿?—õ|"ûÚ?å•(¾®?ªp‹ºP é?ªINHO‰‡?˜o«Úغ?Òy«æUèr?©óˆ?îÇ?î¸Dd*n`?£'Å	1È?qÜژÅÇ?€Ž4¨˜Ã?¢@n¤$A?¢=~áh'y?éF Ô"l?ȅ}'êè[?¶·ÆP<ö"?Á°"rÛa2?¿5@B?¿H",ŽÃ?ì0<˜Y"?¥aƒ–Œ™¸?ŸÒX°xáÇ?š<™Ç
†?¶‰…b¨ù?¡·Fˆ¶?ؑ Jï?´ùÍÂîî?³©'ÂÙ?«κÂñó?áB=ʐÝ]?·ε'ðôMIXED4FGL J1639.3-5146?Ô¤FóÑÀÊÀ
©9û¤QÀ8Z"ÀÀ;0r›þΨ@J(KK?ÿ'%hoU?´Á6þCè?ÓÁêAÞG@ Ã{®Í…@­±~'­¿³1¦–,QÿÞAMÝÙd‹¿Ö]B%iq¿á罞±†u¿ê0[²®=–¿éI˜ÐEþUNASNone3FGL J1639.4-5146?‡GÌ*:?†ýÓã"ùø?퐃4ʯ^?ªí­C?°"!fË?§?uÛ«5C?ªF@Ž­±?­®ÍIJy?âÅXoë?ÃI|\E'?×01¦k94?Â-•åúŠ?Ğ×YvFŒ?ªà‰F1?åyú0Ìë?²Èxá/ˆÃ?Æã@½Æ…Ç?«*FTÂó?¼\&qƒÐÚ?—ƒº-dœu?Ö¸ ɵQl?¤Îªzƒ7?ájÌôÝ/?¦™ú8Qz?…²LI?€XB§‹?í>mN'?¨BÍìÑê?³VLÇX?¦"Sj?•AýµÔ¶ò?™¡ºÂŒ–¢?äžqßZ2?ǾpüÊôä?ֆ£@?î?ÇabS}Î?µ5
ƒ'HH?¥ÐƂä?çAԔJ?µÁÅGµZÇ?É\qêlߖ?°Ôl**?£?§§!¸$?"Õ dºA?×ß­'?®†#€&›?âÜ.øn™Ä?¯<}#‹-BMIXED4FGL J1639.8-4642c?Ö<ë\ž«@¿˜ÉF"'ìÀ7Ÿb¶®}À9,5Ý1žÞ@ }Ö§œ@¸TÛ#§¥?¿÷w›BF?ÂVŠüñ}@";~[O²?÷õY"š&1?½ï¯aOÊ?îØTTëꟿçue!ÂÈg¿æ/$°¹pÏ¿ë]"3¿áHΙ«UNASNone0?ˆyG½Ïq?ƒ®»¿\?}?ÈœÏI¢ã?•,ž¥J?ï¡4K>Ë?š)uâ]ÂN?˜êmüÅ©f?¤_ʐƨ?Ê䎓ä^?Àw$•`Ð?èˆëeX
?ÀT±V¾l|?¬Ðyq˜å?œ¯<þiü?Æeî³ô±?°ÔPúË6?è™|;B~Þ?²M%	Áù?mɹ±4ëm?X"~ôž"?²Q']°Ê?"Æ`\ýU?í˜úY¼¤?•'µOã?z<"1µ)¤?uTÛÀ­Ê?›ÛôjÈL?£UÄTC©?îì§6voÚ?£ÚOhZº?‰¹
.Ilð?"0￞š?Íʓ•&Jö?ÄITÝZ—?è&vñÆMÏ?ÃýÝr¦?ªqñ_ÙMq?—qqîk?ÈÑhä/§?´ž¦…c¢T?è$†°ïݯ?µ÷þÑB?QÂƱÈ?Dœ_¡[Œ_?¸üþ©úÌ?¢£w㺛?ìåý
&?¢È3©uÚOTHER4FGL J1640.3-4917¿ïó‡^ƒ˜ü¿üºüUP"mÀ9(اÌbDÀ:½ž¥rð@úü¹úb1@B_@Ø?À½ÃÚය?Èú(Óo@	¬Ÿ›;ZI@,òý8%?ê6'¾5Û.¿çj®YÒY¿äH$[ÿÛ¿ä«@ "€¿é ¨¡Ê?ª¿ïÿª¥Z—üUNASNone3FGL J1640.6-4917?ªžvy?·ßm•OÆ?Á…,¼Ãâ?¸{²FòT\?æô
Hgø¸?Á@íÂ!?×í´…h?Žaz?ŸLZÏîæ?™ær3zá?ãÂè"ËÌ?Å70ª=?އ"UÚI"?µó×ò}ˆ?º˜wE0áŸ?¥—Kx`?ÚÒMØÙ~?´|]ô|ê?Í&«g™¹œ?¥¡¥ùñ•{?¥~§TÕÓ?ƒ{vv/ƒ?ç^j´ÝJ|?§nø&?°Ÿ˜µ£M?¥.õŒ¹«@?Æ2WÚ?»Ž›"^?è_›«–‡?¾@âât?Á¨®l[ë0?¹s®†¥F?£kO—k?¤G£ƒ'tó?ê_t±Ð?»mîèLý?Ñ1Õ~š?°x†½Ë‡e?ÁI¡DïÚ?¦ÿÆøŒ*?ã3ÕD½?²,.*L9?³ço;Ê|?˜D~íÃRÖ?¬|†Hº÷?'Pe¤?ë»I¸ì×??¡•OoðLMIXED4FGL J1640.9-5853¿åžÌ"GÀ a«°'ÞÀ:*‰*¶ŒïÀ;Å0[žŽ@Õñµd{@Èb?ÍJ|Pª?×	üʃÒ@‡$Y{œY?ÿv"¹ªÎ?珻"–$š¿Ó¯¿uÌ4÷¿ä•"¦óõ0¿ìL<"Í¿áN3i¹Ø¿ïáü^à¶UNASNone?ÜÁÏï¨*<?Ä)Pãÿ³?€¦íÓú0è?u*/lìÊ¿?á\|PĤÆ?ÄJQv®÷¿?ä̔(ý‹?ÄÆñÇê +?Æbùæ?›Î¾;$ôJ?Ö5ª?Ãá'L¡n?æªøêÀ†K?°jp.û»Ú?¦¦3[1?'¦Ê éÆ?Ϫ'""È?®"w1º¸?åÞáæi? .šß+?ªxJªÎ>?‰éc®«C?ÐðŽï'Àu?œß ºÊ;¯?ѬÄà€o?À"²îÄE?…+aIõV)?€3ÌÑ£wô?æÔð
¥±'?ÀÍ>|K?ցzÎ?ÉfÝÙæ*?°À¥í§ó+?²B¦H_²q?â§i?Öüô?ɤÕuE"ø?ލ0—CöF?³*Ñ(Rä¼?²ú°øÀLŠ?šyԚ[r?Ü´#+0ãÖ?³[ÌLõ&?رÜÌIDB?¦½9Þ}aE?¶ô.ŠåM?ŸtiÖª¾|?àȋÈSI?§]o"SøMIXED4FGL J1641.3-2908?ïÒ2x‰e@&—PÁ¹sTÀ9}'šy"jÀ;š™sÚ@¶Ó'7@ýÉÄڐ?¿ª:P³Ì¡?Ö¹;àÖÄó@'Q~wÕ$?øpkܜù?ší"á4¿à£À9 ¿è:T¤MR¿ë³݆Xt¿ïÿpž"ÀI¿ïóÛ._"UNASNone?Úí~ãຕ?Ä¥öÎlÎÏ?ÐIý±éi?À¬a_ø-?Ôȃj5Üc?ÃÃܟd?Äígy-_×?Á뒯3x—?å¯æ—Ï%?Å?ýö)VT?ÄRþ'–O–?½òm_×?Ýe1þ)ç?²;q]ÉÆ?Ì«¿i•x€?­·p²)9^?ÔDîM\¼?°F‹ç•«?Ñ*)²‰ˆ2?¡Õ1­žÕ?Û¾C‹ß¶x?©þ¡Æë‹?Ó'Á–ÁV?¥9jꐟ?ÐBÓâô4"?¦¨,Ѽ˜?֜&_Bä4?űìÎÂ<È?Ù!½Èçª?Å®z/#¸?³ð,RZÚ?¹ÜF£Ž¡)?è40,ÝGˆ?ÆswW5­?Å7)#².2?ÁWËΠ¤?ÖA=ý¼ƒÔ?±P˜xg?Ñ[ûåzSê?±2Þ]D³÷?ØbÆÉ(A?²æŒšæG^?¸;…qt™?•p]Ÿ¾,é?áÞ¨èhà?³|׀ªÁQ?Ö3Îl<Ǻ?±—µ<-ùMIXED4FGL J1641.5+2017?âü8­›"*@Bª\=îxÀ;ÃcTc.¤À<ÇÉ"a:@#gß?ùiþ†ƒ<`?Ë*'Wގ¿£à­Õ:Úq?ÚÃE¤ú˹?ü¡ô;ђY¿×Ɉ'N?è{½`H?4¿Ùu
ƒ'šr¿ÚÅéï'î¿Ùn¾ú|2¿Ç]ŠÊžÊ0UNASNone?ïÁØÀÿm?'…¸#8Ž?@k=ÄIY?VX–õj?}b«åWMf?>+>/+5?ïjiì5{k?•§ç¹Wè?k"QåüØ?y'©íÁa?Ž"p©_^?'òœUº?îûÊ·Qn?"íÚTç?`Bƒ—S‹?_
SDèh½?ž~XªÎæ§?"ÆÇqˆp?í»3GU)'?œýv×?|]×´ÏÛ?hÀ´ï&V?°e_éë-Å?œä­Ö?ï—Bk¬Ãº?†…'«I[?I¶ŽIõ?Däe2h?ˆ‰·P.?…"¬[#xf?î™ñJÛp?¦F¾Gßa?w©+(hý	?"4ÅpîBÔ?£kÅê¾ ù?¤4&~=y?¬ÿÂ?'Õ5
ª§)?hŸÐÑ?gµÞ˜'‹?£½ãÓ+Z?'Q÷p¥µ?é	«åÌx?´t&÷ÉLP?¿ïH쐴?ˆûNPQ?ÉÁRBš?µ*'äM&aAGN4FGL J1642.1-5128¿Å^23ó'LÀ¨…·d†À9¼i"ïÀ:Ý(8-n@"v4åç@_­)™V~?ÒÊ"Ýtæ?àƂ@³½@e¼¦äÜ?ôÇ]_Áq¿ÕþŸb†\ü?íìk΅3±¿èIˆÇì=¿íX›7(‹:¿íÅý¥²­¿ïŠÐsJzxUNASNone?ÏÀA{Aâ?Ãô"@X#œ?¸^Kµ—c?¶L³vøJx?å&*ê—ì?ǀ^KÝš?Í&aã
Ū?ŧ"€zå?Äÿ°[ÊMŽ?¿²ò†ßû?ãv{pÓk'?ÂòɒýÔ?Ôª8(̎?³È ©iŠ?¾7¹)׿Å?¦hGî2!?áãìÆ^Àø?µ=°P q?®ª [O?‡ömÿ^3?ÕqÔc(?©ö¸éɐ?ã\køep·?©AW:î?ÌÀSˆÄ?ÀYy£¯ò÷?Áçó=`?¼ž‰¥R+é?äV&PÅÉ?Åm"€'•?³N¡
?·ºxZ†i?ʍÞbÔê?Åýv5Äæ'?æòÇWdbM?Åå=YÛF@?Ç>e'K=?¬–Àxåö¾?Àt¤Ë.š¦?©^n_T?æ=h°‡?´r1ÜØ?Žþ};?se¼:·ñ?×ñî,Ìob?²¬t£CÀ?ã‹õCìò?²~Œõ\¾OTHER4FGL J1643.1+1436?åâŽm@ .@AuY_í¦aÀ:ÇÌW\À<8Íl.ýD@ßÿ|Øï@;ßY—K?ъ<6\?Êæc¡ºû>?õ¶¥ÉRÄÉ?ðûpú,?ïdH•:¿ç~(kBn¿ç$›?áíE¿æ "@º¿ïÿk*M±?ïú}¹©"UNASNone?îSèY'Ü?¾Î—ŸËâ?¢Ï29°rF?¾ß݂@{?É ¾é½?Œ"Çmsh0?íÊ-tq0?±ñæi"g©? hƒÿ¬Ý"?¨M ²6¥W?¢öÉ%œss?¤ýtó7"Â?ív@EÞJ? O¾eH1²? ðk®¬I?—aœánÎ?§«"Èóo?•UBVۑ³?ì?¤5²r?›ÓRºò`®?¤Íøcñš?Š^´4]QU?³œ\Ԃ¨Û?"`‡—H‡?íOàu?´žù`ÎÐ?§Äh—q‹?²Ú|`>RM?£õyª–
&? ÏÂ`è?éT¤
ûu?ÅqòûN"6?¼°rgë:?ŠÝ6
?º|èw¼éÅ?²(–Qǐ%?ëÐÁµ'Ñ?©Ü†íß/ë?°~ñ¥R?£YýçÝÝ?¶"q¥§?Ÿxàö×5§?æáqä7¼?²©ôB'?·A¶u!´?£_º°Ø‰ö?Ëû«^µds?¯ï25-öAGN4FGL J1643.3-3148¿Ü­³…g!@"|/øìÀ:‹O—ZÀ<DÂ<Pg@9!­NØ*?ÿ?èh3Æ?ʓù\!éà?ۅÎÁC¬¨@‰È]ÒC.@÷é¶9¸?ïôŽýß>i¿çö#]R@•¿ÄQj‹¿ÝӇ;žÍ¿íƒ9¿ïýPÃfò}UNASNone?à,$j\Y?Á8mëÒÚ?ÂN«ió?»‹®ÆÐY?ր¶ñ˜ð?¿1ùˆ}Ξ?ä Áè±ôs?Å`6"š3ü?±×]'Œ?¨/¿Cùß=?ÒH¸—÷?ÃIüD}Þ?èù°Öª¤·?®Vx]ŽðV?¸uâòË[€?£[Ìïa?¿¼–U¹½H?¤;x;¥óo?éG!7ïA?•œ˜*{~?°iä݋P?‰wP)Ê:?Íñmžœ–?'åù(£Í?Ôw×£¦ž÷?½ØZßõsŠ?ÉjŸ¨sÉ?À·]áã­?ßórFf?Á͖vNÝ?Ù܄»;)ø?ÉÜÌòê÷8?Àr{?»b¡³!3?Ýêo‡CÎ?ÉTm¾RQ?ãùq1?´l*§ß²¢?ÄÈ@ýŽ?¬ÈÐg+ËD?̕s³ð¡­?®U0Xe®?áe€Ÿš?¦ÍœÅ6ð?¿(78Ò?¡XìêÊDÏ?Õjðú(¥'?¥>à@–ðMIXED4FGL J1644.1-3055?ԛN·ü@#d:æ…ÛÀ:&k/#:À;žM³9ä@ÙDÿŽk@í£3vO?Î,êâúâ?ÔÉÍéØ?ó›ªà?ÿ)µ@>3—¿ï8‰ÿr¼`?ïò)}§ËŒ¿ìJG¡Õ'd¿Ý‰LûoV¿ë³_¾V'^¿ïùVbã$'UNASNone?ßáWb+]?ȲµȉÇ?žjUZ氘?¢÷'ýë•Ê?ßyR¸oÚ?ÈöL‹QŠë?î>y‹ÃSc?­ÙÓ;>?…ö-gn¥?ŽÛ¾e2³?¦šÛë§+?©mô²ìgL?äûéL°;?±œ—Õé?®ÿ𺸄3?s]Ãö&?Ò(/OŠ#?¯>í2'8?ì[//BŽ?—~%€à>?œoŸ1?|©>k`LL?¶&À¦QM?"ãOï÷?؋nÒµ]ß?ÆÐmǔå¼?«˜9	ps?¦˜¼oŸ"œ?â	/=õY?Çx'ÁkÎ8?ëª
¼,Ó?Áw/Kòò¦?¤]M.¤0¶?®ã+þ%?¼Ô	^?½1"˜E( ?ߛ/ßtLâ?²Š¶•Os`?¼Ÿþøîé­?©€Š9`f ?Ù<ÐbOø³?²¼~ï
?èCBYŽ3+?¬XĨë—?®¸eDyíÝ?•ìdEvc?ÇDÝGÌÐÜ?ª‡¹÷vÞHMIXED4FGL J1644.1-5009¿ïlÅgJ3Àž"B€À9†³k¢À:ïü£T-@££Ùäbk@1n¢u
n?ÓQ§àY?ÛÐo¼@I[»èxû@SóÈF*?³?¼X‹\j?¶8ÐÁy§¿ãRAK#êÁ¿êÞÊl <¿ïñà¸<?ízVs'UNASNone3FGL J1643.6-5002?àáæâu?ǒÜ'1ã?'uÃ%¯%?ŒÝÌo91?Ý&š¥J?Njï¨ÖÇ?à¬Ê¿_?ÅÒôLK:Ä?Ÿ";îGæ?"é–
?Ü®‡†‹c»?ÄÃò™†é?ۀÛ׬¥?³ªeW"Qæ?¹Y¹ñ*?¢v×ÑýR?Þ8åµã?³}T!{Œ?ېÛWݕ%?¯…"4?«ã+(ò?ˆ¨yð¦<?ày_£ÍÏ?¯ˆéš¤5É?ÐûW¦Ò^©?Àé,KYè?šÿjLÝ¥Î?•Ñwûeñ´?æªXÚf?ÀŒÉòÊ?ÉÎÊ0˜×°?Áˆêà31?©'ÙëQã?«ÎXĂ0?çóÕ2vö?¾žÙý»?ÍùýÊ)Æ?¯<<tÔ?»n¤á\?£4©™°¯z?åÀßIý?²©«
?Ãí›côE?¥;÷Ì ?²²tÒú?™¹ÔÐæݦ?è®JÑ??©Ëiñò\eMIXED4FGL J1644.8+1850?ìà2u¦¨Ô@B
Š†×6À:¾B°Ž©À<{ˆÀ-'@Eïµ+?ý¤òÈßØB?Í[JiÑK?ÐÈ b‹l@ö¹!õN@ÊCt
¿ïÛ^g"d?饣'·Ôî¿Ñù1Øýˆ¿Îa
6u¿ênÂÀÚPC¿â—À±5—'UNASNone?ïFúZ¤'D?±ÆÏ˙kØ?vñDJ7©¶? S•hÝd?'dc›Ÿ?¯i…#dÎ?ï˜(v§ãE?…Ê,"ijó?k™p¼nÆ?s˜"©uOÒ?ƒž½Ÿ¥#?{«.Ü%I*?îÛ³"|o?'X?-Ó§ü?ƒºÍu?'ÑøŒ?}<?š¬&Õzòð?‹ž\OuÙØ?îjDw¼û?}λ´~{Ì?'Ä­ßð«?pt¥ceKÒ?ŸòÐM¨ü?u³`$ºíÐ?îÂ'çç?—î°B±ð?‡¯³ðžö?eîüâf?›çá'3¢?"j²Æÿ=?îÔ«[
ê?ôR;¥âA?æ8d
±E?‰ÈO½í?œwxjF†&?•L#|ÙZÕ?í—ÑM:ƒ?Ÿùs?»é?"™]¸²¹?Œ†ò8qU?¬¶<Lîbw?™âaŨýK?ìÃ~Ê,ÖÅ?•E¤•? |""
ß8?‡}±Ò7ªB?±¥¿eÝ´¹?e2—~w¯AGN4FGL J1644.9-4921¿ì/ñÎþšÀL,äd™À9@4ŠKGýÀ:°Ñ®³Ý@é.¦†'@
–»˜Çã?՘L};?ç}®ˆ@•ƒgþí?ú™¨	ôËn¿ïò°Vt€Û?ïýí@
¿ê\ܤZé¿ïÿøsCÄ{?ïÿKÚÉ咿ïÿþÐñUNASNone?ÞÔ?=?Ïäb·ý??´Xïzi?ºÇÓ~AÏX?ÜÀmæ.ë?ρÂíê˜?ÙYðwÝîC?Ð#éò«?¨¿x$"ƒ?°ŽX"]óæ?áÇ,<I?͒#zûÁ#?ÕS'ï[m?²¥¯ÙJTO?Ç°8èR~?®›>È-Nï?ÞÔQ0i³?³1¤cö?O?ÔßÉÝ6Û?¿8÷,ò§R?¼ìûù,ž'?¹&P ú?âYp›ëÐÀ?Á	mňéQ?ÞÕf—r?Î~2Šì®?Á]ãc?À†'Éüì?Ø©!êéöÝ?Ͳ
1e?ÂV\ëÅ?Ä»>OFW?¾©ÆãSÌÜ?Ä\•d?ç•ȀKs?ÉP2¨ëÎ?Íõô¯p?¯ÕþÅZw!?Ï
@1•Æž?³ï0º2?à¿o6n¦ý?´T'%tI?­7‰XŽ?«<êU?ÐùGͨ¦?Í 'C3'í?å¯ìÚg{?̨
ÄÑMIXED4FGL J1645.0+1654¿ìvëÞy·@A­¸<òϖÀ;ÇvK¶¸À<s;ʱiš@á4"å@šoŊ¹,?ÏD¤_E_Ü?©ì^¤Ö?܄YÒÚ-?ÿN‹‰
«¿ÔʏZÑ\Ô¿é^`¨·CÏ¿áØa@Þ°¿â!†BNÚ¿âçÉ0`¿é$UIÞpcUNASNone?ïžq3Jy?w£°D ?N¹·
è'?<~53t?†xÊ¿.é?v­ÖÐLWH?ïôçž	k?†+×Ȩ?fcÍg£é"?h¤—¦¶?‰éÒÎ
èÑ?'²›¡CK?ï_kN5K?{ñýŠ"Ž?f,»T"SÍ?chj¨º{Á?'VÛ%w€7?ym6m‡
?îêšqA?u!ÐHþÀ?jnÙüÌJ?LDÞO·›;?Ÿ^Ö±kv?tY³œšjþ?îè)Ðf'å?"Ptï?`ϸÀ v‡?R΃gWó? pgn"¬L?'Üf{g²õ?îÇÙrnÿ´?Ÿ"ž"…à?tM¶"õg]?}¦¹-IŠ? ø²…¬Ñ?›‹,T­èl?'V08?'T€6¦m-?r†›£€?h3)"è?£q¼¸†‰?Hî¬&¬@?ìÌ­ž6?"At	TL?}s
z÷¡?hFÃô
"?·ÃZýwp—?'Ã
^Ü7AGN4FGL J1645.1-4123c¿îÃò)
ü~@ý+9i®À9ËQ•	ÖÀ;R"nmØ@ â"ÊZW@œ	€²B?Ȕ¤ý¥Ý ?ÏB¨Ã
†@‡p_
¬'?þà-,3Ë?ìÖ`^åh¥?ïâžá78¿Ü=oa·ªý¿Þ3.€›ñ¹¿êãs¢¡¿âüýKð™[UNASNone$?Î_qwœ?¸!«öÑH¬?ž`¿<Ô7H?']K×ç)'?çu¨©Ï>?¹r'·&‰?׶FWAG?ÅQOº
¿?½ð%qº¿?³{¨t>E?àfÙï±9…?ÄjǍâp?Þ^,Þ&Þ³?²"™if?²h·LӅ]?ŸU$ß?Ý¥N6Lv?²7–ƒàUÞ?Õ^PLJ'Z?¥÷Õ9,òQ?ÁodœŒ¾?›ºbP§ï:?àôþu¢­?§ç@%ëê"?·¹Ø+å0þ?©2ƒ9I¼{?¬¿cäž(3?¡–'¯ï±?ë<μTô=?±d˜r1ˆª?ÃR£ÂM©?½þ;â
?ÇkUÑI?ÂxnŸc!?åP›²3Ö?ÅSϾwR%?Ïْáw1?­†Û·,nÌ?¾ÛM¡§Ò?¦BŒ àV?ä]_çÀ™?°òÐ-ߟ(?ÂUì«Ë‡? ä	ú0±n?Æd;§(«ù?©-oiŽFÒ?åѪ
â ?®2 ÁD,MIXED4FGL J1645.2-5218?ÁƒßnÌ!½Às©óƒð»À9¼)DœèÀ;/Ââæ@»ÑOéL_@&t	?á » Ôv?Õ¡}]ù°[@(a´Oþ@ÍüLÂ%?ïüÒf(S¿é1ÁXÐQ¿ë¯¾¿Böu¿ãr®]Ëã¿ïòÔÔK4¿àME}¸'ƒUNASNone?â¼Ñý8O?̧3žp¡†?̛ÕúÚ?ψ¢Í=?Ès®½15?À'à<Á&{?à±òè"'0?ÅXWj—p?£ØÏFÇ?¢¼R¾)K?Ü!Uؾ?Ãö—§ã§?áËhñRŠ‰?²n^"$$h?¹J‡›ÔØ?£Ã.¡$¾«?ÖŒ6¸+‰?±¦¡
+q?Ü)×3ú÷?¨øJ°ÑA?¸â" "¯3?Ÿ˜ââ?ݝƒ¤öÖ?ª4 jò|?ؾì4:™?ǔAYÖNð?Ö"¡À""û?ÎúCTµÜ=?Ñr`0l?Åw`Ô?ÊV%Û^?¬…	9˜?³Áæÿ
?´Ù€ìýÙZ?æòUÃW?ñ1ÀWò?Õӎš.ŒR?²±–d«²=?ÃøÀÈ©ôÓ?¬)ÈéÌ	?à€4ÌC?´j'¼	úã?Åæ:¯Üڕ?¨zUã_«ú?¼	d("¿©?´Ú2"ð;Ó?çDÎø1f?µþÝrwÆÕMIXED4FGL J1645.4-5514?æ2&
À*è},{‰À:¨`ÔV.À;ÇÌÒ¬	ß@HýwÞ@DÄ¥¶ÞN?Ԃ¡z¹"œ?âövÛ)@©G{¿"@Õ†å"?ïç''kþ¿ãPR]šåÊ¿æk_)[C¿ë˘_1鲿ïÿÿ" 5•?ï÷üß¶´UNASNone?å‰"…ˆb?ÆÙ$K0Lp?Ãæ?î
<Í?ŒxƘ޼?Åõ5ûÔ;?½Wloâ3?ãJlO´s:?ÆnÂßÍI?£mŠðO?¦^k©Èñ?Öýv:ÂÊ?Ą]^ø*k?æïíüÐÔ!?°Œ‰©¡?ºãî`©'?¥gPQi8°?ÆÎQZè?©¿I_þ?凝 j?¬ Hê'v?³$
·‰Õ½?'úÇ\^?Ñù'ãI¼?¨æ_U\6?à+ª®jg?Ç
ôoþëƒ?ÊàT/xd?Ä™nGþ"?Ò8€‹;ï?ÄCµÆd'?Ñâ'%'òÈ?Æç¹üÕB?ºœ‡¤h?¾Ë¯€á'Ö?ã̳٥'?ÈÐo¤R°&?ß®çæûïr?µLcÈsÄ?ÇɆÀ½¹£?²Í¨Š?ÔlT¸¥3½?²Þ·4Mÿ+?ÑÙI㽙?®ˆìÏ×?Â;eÕÜ?ª°î€?ℲÇë¼?²J—ýØMIXED4FGL J1646.5-4406?¨3(<ÞMk?éÀ̾µÀ8â­Yiþ¡À:PÑCT§@#úäY€@²¤}"jŽ?ȸ=³™?Ã5֟™?ü¸n;Fýë@ã[:¹9r?ïþôÒ¥Sâ¿å—ñŽM5=¿à',)S¶`¿æj*sq¿èï€@'&5¿ï딾h…ûUNASNone?œûî*"È?'Õvvn?…—'ƒ¡Œb?ƒ†:?îÁÉN›¢?—Ì©ŸÑ¢?¿!k0`×?¾§)ìì?¢¹ÒÎ]_p? Øó/"E?êð5lÉV÷?¿Ô°4ÕcŽ?Ã(eàŒ?¨{:!Ó©$?ºMxj="?¦û.d5lp?çì7±G5I?°Šn&7òí?»üúÒn¢J?œ»ü|6?Ÿ;âõ§8?{éj¨B'd?ë‡vÆ̎?Ÿ{påõ?'Rџt˜ç?…ˆ0Ä ´^?'ª$ê;?r*»ÿ˜Ò?ï"ÁP?Ü'ŠW0?®ÌUâaà?¬Ìðì?¢Aœgá-?¥óOÚûè?ìï ÛS¢?³KÓ!>'á?½¡VU»ã	?¤%Öo·¾?¹0cæëm2?¥êŽÞèsÀ?é%ȸ¯Î(?®IhZÃÒ?¢Þä'o2G?‹»m?M¼¯? §¢9v$?…<v˜Û?íÇ íÃ3é?""þ…k4OTHER4FGL J1646.7-2154?ïýòñÆùœ@-ÑÌÙb…À:°«."À;a_–i@6ãtt@Z¹ÚÁ6?ÈjkØLˆ?ßGX"%"@3̼ܔÁ@ ŽÂ%?ïÿ¶~¬®I¿á£qõáõ¿ãY.¥.ù¿ê!ÎAÒ¿êՀ?€sƒ¿ïþP½Ý›§UNASNone?ÖÞ°cyeá?ÌqzÁ'1?ÁPï.ª?¿ƒ$š
¥?à<l˜ÇÉ?ÑOˆè¶&1?áTØ.ª¸P?Ïièïö¦?Òý H?˓ñTý™…?ı¡>9Ý®?À⬲ûëH?ØM_íüG?±8ÿ5ÎÅ«?Ìduªs~?­ß¬íA3?ـÝå<Éú?°–2	|%v?ÏåEaÅ?¢hnþ`N¼?Öa@ ×,?«x&ú?Ù¬9½C q?¬[ÞçÆ<)?ĽñÝÓZ[?¿	«SÅÞ?ÊZ}§(?ÆX¯é"ÿ?ä9äÅ_h?Î)¨ð¾]?ÑVwÊ«¤"?͞îDc(¼?ààÙEùUä?ÐÛ-Ëó½?ÉÏ«RÃ`+?ßÒ
(‡‰?ѓûãfå?°ÞÑÊøC?е'×ÿj?´"R?ö.?ݶ§	™²?²lÓ?­û(¸'~O?€£¸Þ+»?ßÊ¢ê¿ì?µ¶ðÈæŸm?Ý4ÐF©ÝŠ?´ömÅîEÊMIXED4FGL J1647.5-5724¿äñ`̸CÃÀ˜Á@§üÀ:
·­€×+À;­ŽŸj"ó@¡Öiƒ§?@*~áS?Èz€ú'V?À¾ß8à^?õu°Ðî?ô¹#ØL\Ð?ïûÅs<7¿¿âc'·Ôî¿çº‹·XÇA¿ìõËß	¿¹HÄiüÉ¿ïú¤£|UNASNone?ãy?»›Ù?ÆëØ$]œ,?"KV•ñE?µƒ£2"ˆÛ?×ÈËæŽÚ?ÆPP§"¶*?ä³Âíµ?ÄÔûº û8?þ÷†"³"?'µš¥4Þ?Õ¨"'þ?ÄÄe~?çGh–¹·¿?±ÏÁuø÷ð?žh¤ÀOw?­Šeç?ÏI"á?±Î×L?èfó	fJ?¥"›O$ð?˜U ñÍN?…‡‹oÍQß?ËZä1î9¯?£÷ ¢%É?Ú·g8&Å?ÇÆ¿þ™_?–êáºäz»?§S»X7"?áìõUúTè?ÇK§Ô߅?ÖÙÚ§Uð?È3hå>**?žX¥¶Øš?§wbq–?ãþMê³Vs?Çø
yfÚf?á1€«Œ?µ'5)%¿â?®/ŠùlÓ?œC=±*HÃ?Úì>#ž?µ`«øiU?Ý8àS3Ñ
?²¥iÐ7ß?¬«=& *? èd"}2?ß1¾Å^T°?²gœe̙"MIXED4FGL J1648.1-1547¿îy¹N'x@2Y"9ÞHÀ:'÷†®À< aïß Œ@"tX€Ÿ¢?ûíÄÉÉN?ÄQÚþ"ÄC?¢ÎéõÒ?á#œ½:ˆ'@J†áÛþ¿åµv9B@í?ïý
q؊p?Ô÷dÛ¡Ò¿àä#á0±ú¿ÑWÊ¡ú;E¿Õšü›¤ÌUNASNone?ï@›§Õ‹?™æÆÓK‡Œ?YPɝ­?V3r¨Óñ?–l{'ÛÀ?˜Û¯õ˜ÌT?ï"ìÔîÉ?'}f˪i?Y¯"ëחh?f<‡í?ˆ'XHÀ?4®‡?î¶çdÊý6?"çЇµ?c–زPÐ?a ÷
Q×R?£X*:ã—?"ÆââiÀY?í)Ø
îpŒ?';hªÇ?tÝÑâ\€?`ÞJ^*%@?µcb‰Ž¾Ý?'#˜èBä?îpxû‹Éo?¡‰"U¤Ô	?sLT"<t±?j¬–¼´˜?¦Žå±VA? É…yüê?ïQéω? ïÓWÃp?i($nĸ½?v|¨¾è:?šð¾<½ÕÌ?žr¢
¶¥4?í™q²?¢q¯Ífx?t•­['Y¤?rYˆ°[ޓ?¶yܚ )×?¢1뮑Ø?é3½œ$°±?¨|
ǁ?ƒÀʗ\¸F?wÁ«MwŠW?Éôüæ3êØ?¨"ì91XAGN4FGL J1648.7+4834?í9ФÙÏÑ@CúúaZëÀ;mÔZ_ÇçÀ<Õί%@)K'Mð¤@Y{2¦E?Ӟì>Ø
?ÁñÞªïj?ò^/`?Û¸?þüE2º‰?ë{¥BDH.?çaR*o?S¿é!³äžzª¿©š«½]™
¿ç`{~¿ïþÜÇÔUNASNone?ïÚ­mû ?c2ÀýϹ½?MÛmÝ|À?DŸÆŽ1ø?n‡vé*Ð]?`v£'p1?ïºÛ_ºr?{Ú¦o
ë?Z
­Œüaj?c®÷ƒŒ†?|ÈΧ¾?tOQ÷è?ïg.¢L=?{&ˆFâDà?hE;?f£NÓêy¹?{Î8¤æ?vϑ܌Œ"?ï$˝¼'Á?yT•ð?ˆ¾ç/DSQ?p©²_Õ?Ž1kéÐA?pÁgr消?ïºS=iÂç?s¦eóu†?`æÿ§~Ø?d:)oÜ?zcTވœÖ?mTö
 A™?ï0a9^y?–&C!Ü?q¨¨ìxÒ?~éñ6>?•"i–Öøs?'8ÐTŒa?îèq#aa¢?Š"ً|>?t$·ÂØ?s—y²2<Ÿ?è´)ªØ¸?†ð"åÎÇ?íò÷*2Gj?"ñ}2J?š\"«s5Ø?ŽŠ3&
?£¢CÙ¼v?‹´ hCeAGN4FGL J1649.2-4513c?á¢F·}ú¿Ò¯¹Á'@âÀ8!:жfYÀ9'˜³ÀŒM@šô¥A@ÍãÉª?ÉS–€	¥›?×D¾uñô¥@úúr!…Œ?ô÷öO½¿æÊUŽ§Î?î‰IõíW‡¿äwv#rËÏ¿ì
"¸aþ¿ë*e~ßÙð¿ïÿø]Ê5™UNASNone1FGL J1649.3-4501c8?¡Ør æ?¸h¤íÖIÞ?€¤C/™d"?'˜IÃIj?î¬ñk]Ø?¸ô(F]A?®ß#Å	½?°®'Rè4?ÒÅX½L&?ÂDÔ®ã?ä´V)Á?ÁC†ƒx?³¦ÒHT$?¢óºÉÖR?Á¦ð¢¿Þ?©6èC|ªÁ?é! º±R"?¯­(3ÿ«?v;Ê#¼½?aºRÿ…Ì}?ª­íRm$?¦9fŽ`rµ?ë(Üð'è?¦Þ€cɛB? n­TÿV?Ã7Ēk§ï?'.ÇJ_? ƒVv¯3à?îp+¾
±?Ã]ƒºpdþ?'¤¼ž'ó?™¿ŠÝb?ÕJf°ä?Ǝ+òw+[?äŦ™d?Åìý¨Ñ‰º?­AdÊì8?šøXkÑà2?Â
]êz³?¬ÉšEáÃ?é©RrXÿ?°ù.¿+?Zb` ìԓ?KíFfŒ§?ÆtÐgó›?²4"ü{Úû?êUšµ½*‡?²P¡ïX±ÖOTHER4FGL J1649.3-4441?ÆYgÝÅ?¡Uûà
Â&À8š³zoÔÀ:6¥Nفç@xF(XcÄ@'I†\?ÄƞµbLü?ÛÒF‰QLú@Þ¶¿DN?ñ#3¾ÉSñ?ï$'¯ÀM¿ÓÁþ\緊¿ÝF1\ïDF¿ä8Ÿž–Xœ¿ìŸÖjÛ@¿ç,ÉVö†ÚUNASNone3FGL J1650.0-4438c?eº»Ñšü?f‹êÚ«éó?¶rA˜<&–?¸–S:7ÿä?íý
CŠ?¸¿`P`,?¤iô¾Âî´?¨{îÉzX?ωùØ7}ß?½½§¢¾'æ?æÖâ><ë]?½#¶Ø2 U?²WLp«r? d^–'»ú?ÐuQT'?²+	m¤äŸ?åz†É)Ìz?³>À6Ðj?{žL»Ï?bĝ˜­D?ŪÕMæ?¥Ø:kÆ(—?ê^"– @?¦¡". ?k™WÐ܇?dq0™ÐÌ?¬νñE[?ÀÆùèӂ?ë9¹·=»Å?À4v	²Ž?†
U}øU?Ž]¦X¬¯ð?Ð>@&?–pôm?父¨¦°a?Âi6gÂ?ª\Ì*WÅÎ?˜¿^‰ª¢?ÑnÍÃlѺ?´0²
NŠ6?å¢Ì[–\V?´âÙº­ Æ?^:}
¡›?L7QWjº±?ÈzØÙu|¯?±…kF¯mÀ?éÒ,‹VéN?±©)'G+=OTHER4FGL J1650.9-4420c¿ÒlbÈæÒ÷?£Ú"1`ÔÀ8W-À-À9™™ãktÃ@A0êX£Û@ª¢]yÑ?ÍZ@ãÉ?Ö®F#û²¾@"gÁLf@.Š:ÖëŠ?ï÷õoƒEš¿á^ÛÝáÈ¿â·[ÐKÝ¿è°é¬×d¿ïÿ{@>Ç?ïŽXÐàÙUNASNone<?F20PÆ?§o~Ï$&?‰yݶ*Ô?˜'Ÿl{Û?î¯êžŽ?¬+¦kÌó1?¹:7áév?º"¦žB~]?´Óå{â|÷?°0føxp?ê>B©Pys?½å ©êZã?Àb3DÁÚ?ªÓ«"`'?ÂT'Zc?«'€b
î?çfž
¨¶©?²kÅj×&?ŒôEZåð?{Ñ}O"àO?¤«C³Z¡;?Ž'øƒ¹ý?îA{[§+å?"ïÌOÇþ?'MÙïÎn2?±|9§wšð?'p-¬7?œQdµ@U?îâ·ÉZ|?³vè«lÙ1?£\¢Ó‹1?§^R{	ý?¶ÔKoø²ð?´*A«²k?ëï¬d'=ï?¶""{ӟ ?´+4]S
? "ËèAŒ?ÁžÅí#s?«±KÌcÊ?é1Âèò?°œždÐ&X?hµóýSØ?^wËÄ@r?§è,Íßž?—²ÖÂÊ…?îhÇ?LϚ?˜Ãì/fëŠOTHER4FGL J1651.1-5848¿ïó&äáÀ"Op\‰À:lm¥À<Lï'Êr@eÂõ]¨@`¿B Ž€?ЬbÉù´?æYYø™Ú@l¯c/zA?ý‰oG‹"Ù?é(j¢‹/ɿޘüŸ£I¿à|·áƒ=7¿ïÝEö"V;¿ïøï4Ö¡b¿ëwž!"£‹UNASNone?ÁgÆ°?Àè_XÜ?Íג®Bóð?Áõ
"î—x?ä&ÔL•QX?ÈÀjš8â?ÎÝÌæð[ë?É$סxFt?нŸÄMo?dž,ûò»Z?ßÔíÖe[?ǎ'gŒ?Ü[¹î½|<?²Ù[Ža¦:?Б•±$6?°@3áSÎ?Ó°`gŽ?²Fåïãœ?Ô¦¸ææÔ`?¥Ž‰äþnq?Ú¨7ÑwU?«abÂ5?бH´L?¥²Ñ>"]?³>ÁÀUûG?²ñØá2Sr?ÎE$¤q†?Ã5GÜÞÉ?ææ~y­–?Æmª<ÿå©?½sœ3@¸ò?Â	®Æb¶•?Õ{r¨¥6l?Í|x}L:?á"Ó%ξ?̙™±8éù?Ñ$ŠM÷/?±oÖn	"•?Ö½gÁãÃ?·œg?Ø.Ù
ð%?¹%ûnúc?»âfD¶
?›iiÝ­~?à¯nÚ —\?¶]IH룟?רˆ¹'J"?´†›-¹
ãMIXED4FGL J1651.7-7241¿ÎõøN@«À1§õûmÊÀ;–÷ÎVòÀ<·•XÂ8õ@!MþºÞ?ÿöÊ,œ‡?Ë9\˜q‰¿~6¼ïMð?µW"ðbS?ñå_?ք²?îvŠÖˆ7r¿âì½B–'Ÿ¿ÜÄр»§6¿äM²À²W¿áf—éJ¿Ó®,ƒk¯ÑUNASNone?ï»ÄvçèÝ?w×&lü,·??©'Š?90ÿX³Á?€¡\ÿ…í?wg"-ÝÕ?ï&BþhŒm?¢ÐzmŽ¶­?uⳊLÇÉ?ˆqõè—B?•¾óO«T{?¡¨]ÿ%?ï;8:ìÝ?†Š<8ÓL?f¯¦60?j_1Š,çY?•Ã±]
U?…­)üç?ì©eHH?™×ŸîÛ0?"ƒ¥ð¡µ?k^r–ëRk?¸1…JÏ~z?šÌ4,ŸŸ?ïr íéÜ?ŽO]xÀÆ?Na9Ö²?MT|†+kæ?»R,´g?Yr¦‹ü?í¶åÈa?·œ¥F›ÑÊ?ŠªÄìØ?™½jqGqØ?­ç ¹r¢Á?µ¢"\'Ç?iÃú'?'ƒý"Ú†ã?qPu˜?r+Y÷¢vS?£ƒÿcÙáa?Œ"…ˆ­?æë¬`ñ‡?±ÃóhР'?—›|šEÁ?‹r¤já}ç?ÒvpÝì7?²ÃZ<¤cAGN4FGL J1651.7-4359¿ã-íÞDÈ?ÃsÖuB!À8Él4Á
À:?u –
@†«×‰¿1@÷n¾ú|3?̂®›‰]â?ãD:AšT*@³Bؤ@8…a8ª?ïü7ž|ØC¿×)íÍ:¿Öª9DDR•¿æ%Ž?w4¿îrg'Ñ`¿ïÿšÜ|UNASNone?bÅCîЮ]?bñÿçõ?ɧE¿&ñÜ?ÒZÙ!h?éƒiLRqš?ÒO¸ÞóÝ?¡'®«àª6?¥;?蕃Ÿ?ÆdêR:'?¹¥š"iÉ?éTJ€½æ¼?º'ÇInø ?¨ÐYP&©¥?—¢´}ÿ÷?Ф¦‰t¼?±qk°B̅?æ ²^(?²§OBf
?"qF´…[\?hS¶Ð%
À?Á·Âd$ö?¡dðò%^Ð?ë@JLC>]?¢0ÇÂþ–?gf–í)Õ
?`àÁg»?ÉFöŪս?ˇxuvi?é–Û¸UË?Ëzí¶@29?‹Ø!X"f?"$ðQ?ÅCpH£™?½†]p…­?ê?Ãh0Q=?½l'#8?¢jèCZN©?Îñ|5­?Òj  žŠ?¶ƒpš¬E?å¤A,3ÿP?¶œö/?d¥\ܪ'?Q®RÔZU!?ÔkÛ#p?«eî=Ø3?ë?¬Š¯h?«¤£Ã& tOTHER4FGL J1652.2-4633e?î­»×~xù¿ø¤ˆxßæÀ6ÿÓÚÞˆÀ:4
*%mx@!?%Ó¤,p?þ»Q•	Ö?žBSŒšÉ?˜€k˜¬p?øþiâò¨ÿ?û~"æ+˜Š?É¡î&ä›K¿Ñ(›@¸­¿Þ•ƒÑF¿ÜIøœ‰c¿á–2§9¿Ûdÿ§j"UNASNone3FGL J1650.3-4600? ÿ=r³C?"ICû3eÔ?wU­þuÒB?FÃháõ
?îÁ`̸CÃ?—ØÒÚüçý?ÀÒ¬dd–?ÁV(OCM÷?À0C¿d?¾+I´ãæ?çÆÈÖÿ?Ä+§Åù–?ªy'"ñ? 9&`W}?•@ƒªyMº?H×¢MN;?í®b¹ˆ¢P?¢›«Ãlð§?Â6p?I[?¤Sü`Ì/?¼ƒ®ãu0?¢ib¡Cˆ?çáî,Bÿ?­ºìÎÀ…?¥¬ã^šÑ8?˜[½Õˆê?vÏ/šÏ?s'*šõ!?îw"›Žøg?š"¦±¼?²"åBUG?µÝÚXÁ?¼HZç
?ÀñþąoZ?ê$h´?ÂÝãüÐ\?§Â+ۑeâ?'c–ݏƒ?‹ø¢V?…Øꯏ8è?îÐ↏? 	a¼>?²C©X®‹Ò?©ϘÝ?Á\ŒÑgľ?«£OJÌõ?é`g ðrf?°¤ó&ï&OTHER4FGL J1652.2-4516?҃a_|£{¿ç—MYO&¯À8¶lCõùÀ:GHÕ[ç‡@Ø èØÇ@¯ð£kªs?ƏêÄ.˜š?אջ2ño@'ö@c^@Ç&)àN4¿ë.ñºÂß
?Ɓkdýێ¿á)à¾ò·¿éA 'oÿl¿ìàD]ýâ¿ïû.¡UÑUNASNone?Ž!Š¥q$l?…ñ
°SÜ?›Ö~ivíñ?™rîëù?î¨ÅâU}¾?žr^ñ#?·»ë*ÀNã?³ø¢©ùé?ÂÃi}-cw?²él·˜›?èW¨;¯å?¹ntNÏ?°©ŽLŒ­?›²HH5|M?¼êÀpсñ?¦jÓ?êMv.@ÁL?ªû÷yN?ªãÔâ F?ˆªÔ½L C?½mý–e©õ?–Wܨ'À?ê¤ðp?œF(í%?€ß³ž.ˆ?sü­q&?›ݸÍÿa?šØ"µDm?îäREÙ9S?œ
Ö"#%?Ÿï<Sç_?ž‡LGÐ?ÄûG$'í"?ºOM"Ñê?éÁ´TIÈ?º÷‹xÔ³?©Eȵ[¯
?'¹:öUo9?»¶xŠÔ?¥H'ÃÐ^?êôÔcw§4?¨!G¾Ô"J?f¼7™Ã?tàHò»ˆ}?Áƒd'oa?¢tKÝã›?ë!ŽŒá?£MjBhxOTHER4FGL J1653.0+3640¿ïùÀ
ï@CW‹'¡¡À;¦±RFÀ<ÿ>Dß-"@Á¼.™ñX?ïö¶À›æü?àã¦Î5'™?ïöÌR֒@Šc0Q¤@~¼èS;¿åf3:¿ïo¿ì©õ÷¼e¿´3'J댿Ç–ý]
w¿ïüÙ¿úVs¿ïð²…"êUNASNone?êiâ–Qh?Î|ÓÔíœj?"çÕy?«up¯W?û'¬"F»?Íj¯~æÃw?íH7^»ø?µ¸épÞ·?¤†k€¶Ü'?°
QiÌnÐ?¦ö??¥\HNùE?ë¢X/?ªc%þ½?¢£º¥oö?–Ÿt—/Æ?¹›a8à"?§'"¤ÛeC?ë	y³Ë!?¤?[ Ó­?žº".v?'¡û4`§,?ÀÔïc®.?¢nËs˜?è™p<[®…?ɎDY~Ôû?¡+Ékö›?¨ }`k6?ÉOL³%˅?ÈïÙ8¸Oµ?ê¨'ÑÖ!?Ä.Èý?´K՟ý?¼‹	볏1?»1ríøx?·¬`ã[Ù?é÷4aÜh÷?°d¶®•c±?¤ÎùL—L?™"ו¨žD?Âïp%Vü'?®Ä'"}&Æ?ç8S·Ý?¶°ÍynK¥?ž›Z‰¦þ? {¥Â
À½?ÐÙ¶¾ö?¶Ú²ÍùòAGN4FGL J1653.2-4349¿éØ©H}2?­‹ÛàùïÀ7œƒujæ(À9Žß‰gó.@@éTA÷@=¼>	P?¹{'G•Á?Ҁ¿®Xë@´û'Ã@æb I?ïþ'ÍzÈ?ãm¬átú~¿å—˜mI¯v¿çךÈÙ"¿ì'†!퐒¿ïÿ踻ÐUNASNone3FGL J1652.8-4351?'àBeJE•?ˆÊSU$&?Ô ±~²@?Ï7SÅ5:?å¤&qȉ
?Ï5$ÀåÊ?"ŒÆއq? Áb¥e?ß]SajÂÛ?Ä¢BpÏ?ßqÃÒ'T®?Ãù!ý´Sã?µ!čóz	?§j=¨N?ØÛÉٗ$c?¹R‹8?àíâÈu-?¹,®h@'½?fª^	4?N(¨Cbnð?Ð_'Õe€@?¨X¢,—?çº=DŸ?¨iƇØ3Û?vŽ¢ ˆ?}¢.翯g?ÔÀ±
mÉ?Í·¯µ òe?årŠ9æfã?ͧ¥û¤F?}av©àÒ©?ˆIP½
?á‡	ãÈV?ÉÓiœÚIk?Ýl 8Û?ɶr‹ka+?©¢Vdb@—? Öò÷v?ØuÓÕa|?½©ˆ¤ÿ©C?â*ð®ÿ1y?½ô–»ÿÜ*?Búÿ0È4Â?2¾£Î­ Ø?ÕYƒÄÆ(?µFªQîL^?åN]"kî?µIÒugMIXED4FGL J1654.2-4907c?µÒ	ú4!
Àe¦$ÂW(À9ŽX«'ÀbÀ;8òòÑCT@ÉÅjØ»î@ˆ¸»Ð`?Ç>ž¡@?Ä÷£‡?û˜…+•°@ !ÂG³¿çíeÿ8Yä¿èÛ­À˜$¿ç]Å]l¡¿ã¿FÒLhŽ¿ëe#ÀÏhˆ¿á¬åÁX¨UNASNone3FGL J1654.3-4907"?ët키àu?³V‡èØvB?}?eFùI?tá}¼ñ?ÁBNÊúuä?²ñÁ0³èU?çK»Uè%)?À'Ìãjjy?|—í|×)?vý¨Û؎?Ðö-100?À+3½û+c?ê|"܊S?ª
M+¾?•Hª¦pè?I¢Dê¿?Ãfb×ÝïV?¨Y ‰‹¥?é˜mKÕ7ø?œÉÈ7F%D?ˆ9›¤ƒ$?g}þ¿ØWx?ȱuΟ?œþzÐÈÞ?â<éÈä"q?Ã_tFh?ˆŸڋ?…¢Øh©?Ú}«¤*Ž–?ÃEÅJçË?ܤæ`¾þû?Ç~?Ï×L?‡~ü¿–žâ?'˜3þ³R?áOÜ†©'?Ç­êxH*?⹿;6.]?¶p°@b?¨³Lñś?šÙÜ	=±à?×vìdS?µ_!
®Î¼?á{ãe7Í?­{ZÜ£?›èUëú!Š?ƒ½6Üð?ÛI³ÖdXÎ?¬óÏDF7MIXED4FGL J1654.5-5509?ïÛ¦"ÃÀòFà!qÀ:6ž«QRÀ;˜14@î—\R'G@Ž÷!4-.?ÔU#}³Š?îÒ/w¼Ð@å?À	oë@ĆD}2†¿ßÇ7a–
¿ÙVÁãd¾Æ¿îˆ™A/R¿Ø8ÄA¸Ý¿î?²{è¯?äÝC!½¿êUNASNone?ºò~?ԉã?¹uߙâ§? ²AF¡n?¡u9€
Þ?떌#d^#?½ŽUòꇍ?àbùvîÚ?ÌB‰ÒÒr?½»|öÔ?¼5bfÁCñ?×ò©$üä˜?È
Îe(MÒ?ÞŸÁØ?±…øP:Ý?ÁŸ5­êg?§ÕYñ†ð?Ù!Åg}½›?°üùE"Âq?á±þý÷g*?µÈýÐ?Í<[':xï?³Ã¯ÞªÄ?Ëû¨àçêh?­ì£´äÿ?¸?aÃ(.(?¶XB¼g?³±€Vï©Z?²à°Gq^?êã¼ÊÀ?Àšíg™d?Ëtà"LJ(?ÈRCªàÏõ?ш"{·U?˦~Yw@?à^~šÎ+?͉|kû?Õp·ìÏC?±²Éý㻿?ÆM"VL¤?­spɘo5?ßhº®è
k?³o	ʚr¦?ÅÞྤɁ?´¾ü9'è?àâhž?Å5(ì2m»?ÔôgÛÜ_<?À֊ª'8ïMIXED4FGL J1655.5-4737e?ïj"êÏ°òÀ@xw
À8Ý/n'"šÀ:ö´°¨ª@ €üU¦z©@¬ŒUÜ?¸.ðƒ`G>?'
ÛéË5?ÝüÙ·–Û@|²>¬
:?êؕ›^–¿×þí›ÏSæ¿éÖt`¿à¦"Àä¿Ý@€Cdô¿ä2Wk!UNASNone3FGL J1655.5-4748?ÞíïkL ?Lj]3Y@0?y&@l½Ôž?pA=gŠ—å?àV»É¢Ô^?Ç}"#ý¤ö?æ
ïí8R,?Â¥w?Ã?uãUà# ?z®\zyu¼?ӌ'ÑdJ?Áák»ö÷Õ?Ý:ygcÖ?¶Š"àkj?¥ÉS€§I?˜õÝ`o‹¼?à͋0Á?¶$Ó4u?ä|MKmÍ?§Œ*05?"Ϫ'M?sœnža?ÕºjÁâ/'?§&ï0
E?ØbÃaÇ£Ì?ñrÊ?"êtësÝÇ?w¯ÛœÀ·ã?ãzô{E#S?óBÇ¿?ÚÚÔRä9·?Æñi8±U?|©×!ö.?‡é"î4µ?âYC²Ô x?Æ͹­LT?Ѷ3>'
?±›"˜¡Æ?¥0ؽ€Z'?–pý¨"°Â?åÑØÕ4£?²=Á9mJ`?Ù"G¦?°QÏlČR?¢ÂU'@÷?‰E¬¤¼¢?âF'*^ß?°‹º)yNŠMIXED4FGL J1655.7-2411?뇚<4@'ºYÀe¶=À:mˆXÿvÀ;áÐ>qT×@†+<™¹O@GE‹$Œ?ÒÌÌ¡Ù¯?Ñ}	@¢C@kõQPT¬?ñÙ5©Eµ?ïþ;9'ò?©2­ý(à¿éYe5
ÿ¿Ø—9¢¸ý¿ïÿë""i·?ïúY,ÁÿêUNASNone?å\l]Ýg
?ÆÞÁnUy?œÎѨ·kR?˜Øé
§?Óz:)'Áw?ÆӏÄý?êTÆΰýŽ?Â1=ÿXÕ?°pŇÊ,?°ñ§î33?¼é"|à?¼šž@6?Ç?è?6,Ž‹?­4e/¬+r?²×±Öqÿ0? Â¦ƒ7Ÿ?ŗNc˜ß=?§û.éZH·?æø'V•t,?ªy• ÆƏ?µÙ€ÇCT?˜þ¬aÖq?É0öåF¥?¦Ìk( X?âšÂ
sÌ?Ç´‰ª8MN?³
îæ:!³?±FNi=²ó?ÖÀ ʃz?ÆÁVCzöc?áìg$"ø*?Î>«y}´?Èi»|å¦?Å\›ò›
?ÐüÙ7œØ?ÇãÎÚ»o?ã2±X'3?±äl$ç!)?À–¬ç?§z£!g4Á?т'Gï
˜?¯.h¾Èaµ?Üê4è¦-b?µüÞëx؆?ÂV~œ"*?®½þtVía?Ùê‹ÉC‰?·KÐ²uäAGN4FGL J1655.9-3940?ï0úÀYŒ@@®I#`À9oe5
ÿÀ;
w?Ò}ç@Dl›ßš@ۉC
@Ì?Í58[' N?Ԟ$c½ù@%XdE#ö?ûqo´Bè2¿ßÒËÿÈLµ?輸dÉ®4?ÓS]Æ.οæ7ûþé¿ç®¤"‰—Ä¿çºßr#UNASNone?Ðzb[-¼ë?ÙiŠªŠÐ?':L…~T{?ˆ¢©9?ç8ümÏ;g?Äd½]²Ò?ÐC×R")?Ä!Žª-X?Ký"z¤?»p/'ŠÞk?ã:,l.ã?ÅXÚ©¯;?Óq8'ÿ²¹?±P§ÜÂ'?¹=q|t?¤wœ»­®?ã¿Çð]å?²'Ć0?ÓLlµ_ó±?©æ"e{z?ÀŽÀ׶?£c—‰Bí?â6ŸßÛ?®÷`¬Ð?Ââ'mµÁ?´Åä§ê'?šÀ<–jWe?"@ãÃvq?êqYßD…?¶ÏS©?¾·¤­°
5?¹ØË¢o?ʪc»ab?ŨñRŠˆÒ?å~r†Û&?Ç[Œ~åŽ?ş-;fLT?¨^²Ýdc?¸›_‡†
ú?¤½ž–å|u?ç"ÈÀ^æ|?°ÉJP	‰?ÁýÙèœÀ?¥¼x¿[?ÂØ`‹¨a«?±Bé>àtü?æihf›Àe?´£yìPçOTHER4FGL J1655.9-3101??þ6–@šºŸ¹À9óëƍ«À;•ËWÇ@Ë…$@22'3K‡?Êáž@zµ?Òa]¿îî@YP%²A0@ûÅÜ¿ì]ä·¥?ï¹ý‡»¢¿æ!;¹êqù¿çlÁÊ:K¿é|0¿ïø0þ¥ŒíUNASNone?ÙÐz+j<?ÃÌçÄõ½Ý?"D]¦2á?‰_ÖO8•?âäöÐ4?ÃüsÈ=Š¿?ãj"ýcÔ¢?ÇöíBõ.?¶L¤4²w'?³>Cè¥)÷?ӗ¬øy¬r?Ä87ÊÂ~?ã‰w€1?±Öm
L?¯—F¨çÝ?™ߌmF?Ö'ôeÃ?°Ôâì…
'?åå¨é÷2°?Ÿ)Œ¼˜•?º
è.…­?"t@/FO?Ëcè@à^¿?š#sãןF?ÆBù&‡i?·÷!e'r?¤¢^+‡×Ë?œ
ôg~©?é%Óp*
?ºŸ3G¼=o?×A­c>Ø?ɵïªa+Ù?Ç5×vã¥ñ?Áà4dï†?Ýbҗ*î/?ÉåôXi›?ØfÉtõí¥?±À£
´©?·ê0;ÛC? Ê'^1¦¦?àØÝÿÐe?²0d
%}?Ü|V:§ÏE?©âu)?Æ3×æäْ?¥²RJ:Ë?Øi½Òø¤±?©b¦2A6OMIXED4FGL J1656.4-0410¿çÎg­Ÿq0@7.¡ ÏÀ:µ¼åÎüÀ<Š
RiY`@c
ÔoX}?þÛ£"Ń?Ì­3ªQx?ä) öÍ1@X§ç:6]@+C&E?ïÿ0,µÿ¿ç9Ù	ññJ¿œ9ÄØó²Ñ¿âž€ô‡%ú¿ëS—tü+¿ïü½àö¥cUNASNone?å^X±ò×?Â;J³d¤?Ð{¡¶ôs?ÁªÖþv_?´©^µLez?¦°¾	¡¥"?äKŽž¾Ç{?É!dé!?Ðú$¸Šå;?ÆãFmvâ?¹ºø#'¬@?±Ce8‰¡c?⽀Ȭ"?´üþ%›?Ñù¡38^
?²"³ú$?ÁºvÞٕ?¦QÙ¹à°?ãÖlÓ_Z{?¤	VÊIâ8?É,rJ†r1?¡¢ˆh?ÇyÚgü#ä?œâJ9>wû?à\/¡‹Þù?ã\͸?Õª»ß
Ü?ÃÓi«§?Ã9ËHhb?´¶s.2ÞÉ?Øäl8ôÏ?ÌxWðà?݅òÒ^Ë×?ΖyY¿?Ã+Aë:~µ?·$-"®jƒ?ÜϋàB?¸5'XÔ»?×Ù+òÄz?¹.Ÿ0a¡?Æ®'ۑÙ?«±áH‹³H?Ô¡õ1´œÄ?¬Ž'¾-øŒ?Õœaä»E?±×nbõrÒ?Ö@nmyˆ¶?­aØ0»MIXED4FGL J1656.5-2733¿ïÿúÉVÂý@#Zï
å6PÀ:ŽP±É;HÀ<pSó.@ªvºœs"@kXZ4?ÍOʘ•Â?éäjþ{›'@4,ºËC@·dÒ<£I?ïÿ0ýñˆ¿è‡¤Ú?|¿³çÆÎ0$5¿ç¬—7¿‰î¿ïÿàŽ¾¿ï±g¸ÎéUNASNone?¸>J}L"?¶uå6/z?×7<Ynþˆ?ÇÞxŽå""?á\ž)ÝZJ?ÈÑBe³Á—?Ägð4>?Åm™¸š³?ãø¢û0ý?ÉX=÷ºê«?˵ƒß6ö{?ÀÙ·®¯?ђ¢ÃӘ³?°ì-x~Õ?àf_€]?³]ˆ™`?Ë@yþÚÍ'?¬d•Dº?ʔ€fSk?£æ݈'?âÐÑxÐm¹?¯LÛFnµ?Ê(9¶kG³?§ÒþH¨Œè?°›×³ñå?¯'Ï'Ó'5?×Q²ÒG,‡?Ç¢£ä P'?âEsh`?È&Зe?}?³ÐÉ	2?¼£±""ù¥?æH}þúê?Ëy_èÉ?ÍQ#˜$hY?Æ%ž	ÀÉ?ÈBCwàœ?¬ëªÜ­­‡?â©´û†÷?´Ì+ÅF>Õ?ÍèšӉ?°…æé(" ?­FFt#U?"L«†ž?æV×â}>?³ÐåY¥3?ÏSÛ:"ç?²%~¿5¥øMIXED4FGL J1656.9-4814?ëÌÞvÝçÀ	½nŠø'À9Ã;òõU'À;[;¸Ìe@UM–
îÆ@vßîÁ?Ö;Y½‹'C?ïNÀøƒ3ý@	 Vßà¥È@‹~M㸢¿ë}	@¢C¿ËßýV,‡r¿ç%IÑiò¿éŸ}ß(ïã¿â+úú݁P¿ïò¾UNASNone?Ýþyµ 	?ƽ·È'Þ?‰Y¸g–æW?€¿B3¢âø?à›\Cf ã?ÆÂÅï°I?ܺižæEÖ?'câÂFP?²aHú'®?±ËôÌö?Þ¢>¿œŸ?È+V^Ë+Q?â…Sw)	í?²®ñZÏ"?´ZþÊ,? ç&dI©ã?ÕÞÓÊíÏ|?±´@^]ç?àÁÝF±Y?±¨ÁO4(x?ÄVxª>ì?©¬Ÿß£?ÔQ	œ.[?­çHœM"c?ËÇ|z:¯?À#É!¶Lò?'Š
©}ò‡?]ÆVQu‡?èyÐ¥c@0?À¯ˆ}V[Æ?Æ÷ïè
y?ÄÓ&¥}Ÿà?ÁX1šöš?ÁM,:'ðU?åì+Àß>û?Èsše‹8ò?֛ìm"›c?³jêÄ)q?¸à‡±éb?£ƒ§ö ?á•øÒåÂ?´E»r±?ˇK²Ê±Ù?±ÿÕqƒr?ÒÖ¯G3xÜ?¼q{ËÛé©?ßeªßg.7?º|RvorÿMIXED4FGL J1656.9-5717?ǾHoÛZ.À!¤Œ?>qÀ:¬TƒåÓ.À<+óV¤Q"@=lè5³ì@ij­?ÑAǀ\±²?âȘ?|l¸@,ûõ@þè'¯q¿ï¾´ -œñ?ïï* ­Ò¿âî1× ì¿éHÂ:¢"¿ìŽöþN¤ÿ¿ïÿ¦¶tFUNASNone?ى‡Æ»ï8?Âß=45^(?Ê)õã­ ?ÀîƒËüî(?Ùa}H€!x?Á¤v¦iO"?âepz£?ɬS'p§Õ?³2~¦zÝÕ?²oDP/B?Ö–"Ûf?Ç>ÑÌæÎ?挌Œl?²àÀËÔ؟?Ã."6Þ?­"¥çÂ8?¡™@¿t?¥ÏbÛÙÄ?é]€Z­î?—áJ`Ÿ?¸a¹«`U%?'+8™Í¼¤?¼²C…Lé?'åU´ÜN?ÆËËtKñ	?¹Ví0´Aª?ÑÆu'žî?Æ×鍚)Y?áiÒaê´G?Åkå)B¢?×fôàV_?ËOèD;]?ÁvyÊ?À—¦îI|Ô?ßÊd›=¼?Ì¿!(wK?Ýú˜{Ñ!?»ß.›–@?Óüž²Ä?»puo)Ü?Ï·òÕÊø6?°è•íFý±?áõîÓ¡—?¨nÈïúM?È1՘«æ?¥ÙuJÜ}?Ïöoͽt?¥j¾¿â¼JMIXED4FGL J1657.3-6232?èç"oL$WÀ(+{®ÍÀ:jª|?ìÀ;Ódύqm@^BT8fy@œ÷_GŽ4?Ê{mI.!?¶XYÞBÀð?êÂä`è">@•¤"^¥¿ïüÏ(ǟf?Ödü¿â	€²B¿æ™Y_ç¿éßv½Ì~É¿ë{j=‹|UNASNone?ìæÑ|£®_?º–ïÛ!?õ8ÚD¸?l£òW?µUuíì?·ôF&׏†?ï{ìàñûc?'] äÉe1?^ÄøšÁnî?cøjߘ¾•?,(¿÷-G?'c ®ÍI?양î:ÁÙ?£LuFf"?"náEeöæ?Š›Lžªº?¶o¸>ˆA|? Ò¬
º?íx£Vÿ²?‡f7x"z?‹†¤¹!8?lV¿±.¬S?°ØÔs'Ç?"÷È'Úˆ?ë›lÖ[Ü?½éBãM?›Îç
9	¤?˜VŽ¤jz?¼4:ÖPë;?º´–Ü62}?î‹$5?ªÁ2<ý²?z1Yì;ò?Œ¯ãKÙ8?¤
pÏÔqº?¨ªÁdWÑ?èµJYëXÔ?±ÁyttÂ?£õVëî?"¼CAè›?ÈFÙBÑáµ?°?ç=|½_?êPîK÷V? éCsCÚÐ?›Þ€NP`?…ÍÔ^¼xí?Ã@vʄš?ž¨"‹¬\AGN4FGL J1657.4-3917c?îÿ°­îv|@TÔ#&vÀ:_©³ÃÀ;ŽÚLè@Ç)_Iç€@±'!ûÓK?Ð
CàT"?á¡b§K3@	· QºÞ?úÖ=3'(·?ïùh6J>连à7|‡Ôº¿âYl¸K¿åßbцoñ¿æÃ^)+¿ïÞ´ -œñUNASNone3FGL J1656.9-3919c8?Íf[¥SrT?¿85P™Ën?'<ÁÉ°Úö?ŒÐØ$bÖ?èƒäd?Àsº±}?Øo.{éZw?Ìn÷(.â?¾×1!,—Û?´‹ï÷oÚ?ßÛ:¸žÔ?ɱr©7>?ړ@;âã?²ž
¡Z+?³›)Ÿ]>O?|üSBà4?àC«ˆsE?²Û
ñ(Tf?ÔdÔäQ? íY[Ò=ï?Ê8D÷Î$³? ŠÆ©ïÅ?ÞŸÇí%?¤Î®v»í-?º¡¨‰á?®»«lÐÍ?£±µPK Q? «Ñ2?ËÑ?ëpÁV!ß?³.ºz%:@?Áþ&æ7›¼?ÃgüUGýg?È.õ²…_?Á"/Z"(Ê?åt¸ÙÐÁN?ÈAFßÀù?̟'Ë»™?®
E¼c‡?¶Yn ¢ž?¡/†qÇä?æñŒíI?²À"?Q?¿áu«ëè?™Ñ•Gg'?Ð0	q‡›"?­Š<(_ù?ãë̥ƴÁ?¯yè6PB9OTHER4FGL J1657.7-4656c?ê¢
L™·À&"»À9$¯öÓ0"À:̨¡tYn@X=EZÓ
@ÿb›ÖŠ¼?Å3{''PÓ?ÀG/~ó¦?þÙ&ýšÊò?üÀ¤ ]Øù?ïß:Þ"_¦?ê÷Û8 Z~¿Ù™»þHoÛ¿çWšPx¾X¿ßÑÃ×/Ò¿ì*© öUNASNone3FGL J1657.6-4653 ?¼¯óšŽX•?²çÆ3'¹?†â°ÕC•‹?ƒ›Œ¯AžË?ìvÉÇ?³Ž–2[?Ú@™P?Å+\bŠw?¡
'ú†(?›¥ÜZúƇ?á㾸¯Uæ?Äy>"ƒQ?Ñΰ·ÃPL?²OhŸv‰?¶?´¡·ê?¤kŒ¯Àk?äP±×v?³–á
¹‹ƒ?ÒÞô¦c4?©)ˆtå!†?³ÀÝ0ÙM?"ò ô`Ge?äòê³<?ªÎ˜YY?³(R:§Ÿ*?¦ épÑ·?'à˜!Bœ'?j›'®Ý³?íð÷"8Æ?©úZ_ç?Åé1𛑟?¼³ßåz»?¨·Gé‡?©ùlpŸ-
?èú:hý?¾0˜¤&:|?Ã;o{Ò£?§<¦B'--?´¶zc¿G?£A¦{oÜ?èšTÔ\|ò?®cmÅjN?Á*+ÇùO?£ú*vGÆB?¸nÃgµ?¢O×Ê$þq?è´çJÒa6?¬fùyÍ"<OTHER4FGL J1657.7-4520¿ÑRPæ~¿øsÓ¼«šÀ9>0vÀP¾À:´ç]7@ \oço@ÿ¾¹ä'¼?Å9ügÅ?´»1CïÃó?ìr9¾g¯<@%e/.Á´?ï	Zò"Ý¿ëݟM7Á7¿Ív߇ϿçXࡕç]¿êÂìÿr;‡¿¸Ï¾Ä¡Z-UNASNone?¿¦ÒŽÂv?´
½'¼'?ÜokÃ~?‡Ü³þ'k\?듳é¦ø'?µLÐD#æý?х±I'€?ǺòoH¸+?'7öÒ´â-?"ï1m䞠?æ«g¤ÿÔ6?ÇZ|îh(?×\Z_ƒ."?´"Ñ:$&?°ºåÈ
?ž,‹iÏ(Q?â?Ûsië<?´Ž³Db?Ó²¤ÏÐ?§9ҝfð´?"Å'Z‹ä?vPQðñ@á?å×Ó{A?§Umî
®1?¬*¤âÔÊ?£&­;RŠ"?¡ÃY'Šµ?‹†q¢i?í¸HÛ)ö?§9ê{l."?‹šåkw?º;>ý8Fæ?O®Ç†Å_?š‹PMª–?êçþ(Š
?ºï£w¥S?È!ðïۉm?«Ý'{ú?±ƒZºw?
$Êy[B?ç×Xˆ"s?®÷»Çmœ£?»D!­T7?œïf2l—a?™‡Ù,æð?…»ªõéO?ëËCó/Ò?ž±ÂreTOTHER4FGL J1658.3-4637c?ä͵ˆ–ÀDoÞµ,À9Zgä맃À:×qºWC@ Ÿê§Ê@‹˜AªÅ;?Çð½Ø=CW?»`õ
]¶"?÷­íCdٞ?ö¦+'Ëöä¿ïþ°nÈ5?ïþ`ù?Ÿ¿èýIúÑÿÛÄQ¾Ž›¿ëüº0ƒ¿áü\§ ÃZUNASNone$?®`€xPj?¨[úHMO(?ƒ¸t]¥?†CÈ#<<"?íË&2×?ª£ K¼üQ?Ó
@[öÝ?ÄÁG'ܽÜ?°U#â¢ú?¬v\ 
ýÊ?äoVc}'?Ã÷À^‡þD?Ñ­¢"‡Çé?±3êäÌ4?·ì«hOÔç?¤Ê(AXF?ä+™¤bÿ?²®s²Ÿ?ʲJf;Ú]? ½¿ÔìP?»L»@C£)?šÎDé`x³?åéÕþh•?¤š-x•/U?¨Áæ!µò?¥lý)¶Þ?‹–GÐZ=<?‹‰~ru?î\{¬?©Ì1T2s?»¬zª–?¹…î#Ü?µà!n]ØX?¸ùc");?éÒN'y?ÀԂ́+?ÅÓÏ­IF<?©¿áéÕÌD?¸<¦)?¬?¤wöˆ?çƒyÿöDë?¯ÏŸÏäe?µTj½…~|?—®Ä|…Ý[?ÀÏè§!‰?¦°a'}[ï?é!x~IŸ?©:Àx0‡OTHER4FGL J1658.5+4315?áè–Ž*@C#£ÂÀ;å§Ð"ªÀ<ý»9ýQÐ@!Ѐ2ë9Ê?ÿB0[è^#?Éq*º"º2¿¯ðZà:+º?à±&~
"@ßÀÅW†¿éeì"ÓiŸ¿ïî>ÅèW?ë	IàsÈ¥¿åMtýØÞ¿Ùd^—ºò?ʔG_ºû"UNASNone?ïÄ9œÈ'î?r%çþµ?C'¿N?7/ç<M?{pÙ¼‰Z ?qfš"o{÷?ï–^E}/?× Uïw|?`õCU©'?jG¹eY{'?†+Ó	-Ï?‰ôü˜vÁÄ?ïIþѓ?Œ@ÀŒ
?`Eì™&õ?bèSÅ0‡?šÔe%&]À?‹Ÿ|6hd?ïŒè0UˆH?t1vòßä?F™dë2Oî?@tæ&S?‹\]£õ;?tb[ñ–¦?ï}͗'ÆU?";A¯UÎ(?Qê´ºjs3?H£Ë'‹@?ŽOClI?ƒ‡×'<Ã?ïl²Áïà?£ãeÉ2[?j4š†Žg?z¬l!iƾ?œkÖ_?"!?¢¦¬1ä¹?îeƒõ9õ¼?"QKº",#?eš½âsÞ?eËâM/?¨NÒHWu?"ò¢ì ôú?îNàÀʊþ?—ð~xn
Q?_\ÖÒU"?a	Š ·{ô?ª!tî?—¾äÖÅ¡AGN4FGL J1659.0-0140?Ø_ŸðL@7큾±À:»df²À;ÛVSÉ«°@6ÖS3XÈ?ý«m6d@?Ə¿P7{?Û¬D6¿@a¸¼-B?÷ÚJ><¦¤?ï ÊæB¿˜¿Ý ="(¿ÍÄüžÌ‰[¿à^ý':пïû½ü?ìôêÃùUNASNone3FGL J1659.0-0142?ÙÑüò"la?Äý½‡¬Ô?ÓQ—^"m?Åhð]º_&?ÒÜîvq3?Ã,vO+{?à	·\­¢?ό³4ÓÏÔ?ق\"ä?Î]cü\e?¹©údà\?°ñr'J?Õ¶/UÇÌw?²ÝlqA?ØÍrr÷¢?²ÙYÂÑç¸?Ñ|^˜Å;ç?°ÑG$¿˜€?ÚFCCª,l?¬›Ëþè?Èë¢epH?¥V$:L "?ÙC뉝Åp?®Ä‰Øí}®?Ñ kG9Õ?ÁÅlL?¯Ô?ؒ"E¹6‡?Ç4…¶ÁPJ?ÕÍs.¤?Ĭ"Z¶Ÿ?Îf9±~N?Ëd£KQÁ?ä@¹°²²<?ÏêdL·?À–à'ƒ¸Ã?¸Ï¼.X¨Å?Îœ
áŒ?±H:E:
­?ݲ?'çù¤?ºk·ž'QÒ?ÓArf#öT?´¯yd¹Ë»?Æä,ü?§.>i¸¤x?Ï!'-áÜ÷?³'"¿¶Ë?â~pÈa{?·'cý­ÐMIXED4FGL J1659.2-1443?î°¥¢™ûó@0ÉõœÏ®ÿÀ9úú0³&3À;ڻݑ@/@ô%ø¸
"@‹Ù½v?Ȉ}£–s?Ó^lÇÔ@} >ÏI@—†¡ð*J?ïýW¿.©Œ?ÐëÂßä¿äTŒÿØ<í¿Ùª‡Þ0Ly¿ï['\¼?åF>QÊMUNASNone?ìÞHd•"^?°Õôœº?'î$x«?"^'`Å?´R6ÐîçÌ?­i¿éèÑ
?î,;s"ˆ?«*¯Äè͕?š¶ýR‡©†?¡üT,…¢Ÿ?ŸÁžùÞ[s?š[þ҅'Û?éÖâQ¸Â?­<ÛCÕd?¯ÁH%±àû?Ÿr‰…E?À´$°õ'ù?§Ÿ¡¿¸?ìÓæ7	µ?'W­2u¡?¡oyûèšé?ƒfÞD?°©I¾	ò?‹Æ-#ä1?ê™êDVñÿ?·Ë¶ì|?¥ñ'/aðÊ?£%RLO¼?Àöb"Â?´¡ÿB搊?ëlìàÇE?ÀR23Ñ54?±ÀÁ$Ü?¹+n¬[?²Ø~7N±û?¬;B®ø¼Å?æAüKŒè©?°¼Iºç¥Ÿ?¸-úªÀ-?£ qVÝÆë?Êá?Ô		È?¬Tq™»Ìv?ç»ù9–?¨97¬…'É?¶'YÇ7/Ä? %ª ²O?ÅÊ{8ÛhÇ?£0ϑßL<AGN4FGL J1659.6+4918?ìém,B@CpޏlðÀ;§iϧr À<ßjT1°|@"yÅï@ÿÿ«Fj?ÓZ]āNÊ?¼.)‰_?æ×
˜n÷/@œ=D:¿íèØÁ¢¢,¿åP³a@➿àz=|bQ¿àœýÒ(V¿ßå»[5ZÖ¿ïý(_D´UNASNone?ïè	r£?W2]z "?9óò»»hl?-¼šÖR®?d®xvWp?Tß"‹Ui*?ïÄø:
íÔ?unڔè°/?Ln¯oz?S'¯C÷?yöÿO¡?r³_ÍäI?ïtRªz?~Í9ì¤ER?_RÚ|'•?\‡Dê' ?	õ-[[Z?}¸ÙHXÐÑ?ï»ãތ<å?`Ù^o
â;?MbRсM?40qï j?~aÆz•uÝ?`OÎeNq?ïѦ¾ù®
?føÜýöÖ+?E$–J¢@'?6Ê&ãe?tˆ
˜Øs0?e›BñÔ?ï[ñX>Ó?—xºÎ]÷?]Ú¹w@
€?h—¸À¾³?'Áv=°ÿ?ŒÈK/iª2?îÛRû5Ò?|}|A?iŸ~†%òü?d˜DÈB? °ØcN›ÿ?ŽÎD¦æ?ï'l0ˆfŸ?d[ÿm#"?`}EǨª=?S…;yŒã›?™Ñ9ŨÔ?*ÀD
AGN4FGL J1700.0-0122?ç@h¼h6Ü@7ÝxqOÎÀ:oSשÀ;Ä76Íòg@Aº£@°'w"Œ?ԗg›ñ
?ãÁ1"·ºí@
çööl@ys×=>$?æA-ô/?ä˜`‰' ¿á…²œøŸ¿ë¥<e¿íÁ¼-BXj¿ïþ/EgéUNASNone?ã`Œ~—ÏY?ÂÛÄ÷ÁB*?ε4¦at?¾ÀÞ[Y[Ö?Ãș_?´)?¹Æ— V?ámg›H?Ϩ¥'c¾Ž?×/l ±ó¥?α¿í¸¢?·×¤\-?±Ý½_"ey?á[èoP×?³&&·þM?ÇÞ;iãs'?«9.Ãä{?Ò*z/¤'?¯÷7áA¼?Ðñ;²š?£ùûÒEs?ß>LFZ,?¯YyklXÅ?Ï ñèHr?ª0qÖ¿¼?Ö$…jƒ¤?Âtw€ê÷?ÛÖ Ý_
?ÅÅÿþþM?Ì
³*lîž?À¾."×?Ó@–oåãl?ÏÕq›­–?â‰ÒÝï;?Ñ"à@g?¾¯Pï {?´Ÿ›D<æ?ÖßG<™R;?´°bD)?Ò½h\F
<?´Qµœ)?ÖcPg  ‰?³Hhâ²?³÷ÕCé¹Ã?–@‰CFaõ?ãw0y«£Ã?¸¬Ù_©Ê?Ô©¼7ºh?¶¾+ïþó>MIXED4FGL J1700.2-4237c¿Ü»­ù€'•¿É=4D«+À8N>X*cÀ9ñ²½W@–ë_µ@G`Æu?ǹNè›_?ÜnÛëMÁT@d öðŒÅ@ˆŒxô³q¿êâ‹`òË?ïüJ~Sm¿å-݈ܳ¿ì Ñ0à¿ïÂã>ÿ¿ïö'=¯¸ëUNASNone,?§ ´{SO·?¯i›=øLò?Ép&!µ"?£³È‡ØKè?헩6ð'	?³Ê *KÉ?°SЬhCÚ?°40~åô?ÔXõ™?#?ÁŸJ!¯?ãÉ)SáT?Àf¤h™`S?»÷Ðñõ{B?§Bþn½"?Á3¹Ë";Ü?¨CFºo?7?è4nSA?°a«ø÷
)?™ñ"Ù+?€PèèÃQ?ÇÄIà7§{?¦
æ`¯?é?dvø?¨ƒÇ¥X?‡"¾Šâ'?‡ãFU•W?¡
[PB>'?¢M¦@ºèñ?î'Pù?¤É1ºF¿*?—ê2X¶³?–ÒIKi?ÖbJfÅJ¼?ƨF"¨²Ö?䊋xˆl?ÆE¢ßÇ?³'ÙLõˆ? ¸üyµ™?Áƒ…ïKZz?«fî.+?é:#Z€²¡?¯/_·íå?&Ï妜?iûÖá\×?Í,iÓ¶Ôq?³ã*Ú!³ª?èv—í$¹¦?´F%Ö¸ºÅOTHER4FGL J1700.3-4557¿²(õ̯ÀyãìëÀ9&p­FÀ:ŠšÔ,<Ÿ@ÐÁ{µØê@#Ɔa®q?ʘÜñç?πåÇFü@c›{)Q@¶•bþ'
¿å‰¡iq³¢?ï†Nc:aü¿æüÚQοæjqáÕ¿ê4{'W]µ¿ïþêÁªYÛUNASNone?ÙZ2"Ÿ??ÂWsT'Ü?²¯»ÐîH?¨,£X&‹?á0¿e†?ÂƄko?Óۆ	U$†?ĝÀDÔ?¯ãîi?§ßàaë\¤?ä!>¼SWì?Ã:5äqä?ÕÑêðñ' ?´=Xå,;´?º×™;r>X?¤o·>\ß?á¼`¢_Ä?´RÂÈ œ?ËRþÀ´? Hë!
Ñ+?¶—+ oU0?'Áqþ¸j?æX[A©Ý?¡§I»¢èT?È
Úwôòõ?¸vµ'fd?´˜ÃTÚÌ
?«9Ο?çip÷0p?½Š>̈H'?½†Ã­X,+?¶I¾ïLP&?µÛNxf¡¨?´"8l1´?铽»H&F?¼ÙJQ»g'?ÅUíku;?©«5`Oš?½äû,[¨?¥†úW4õI?æ?°0ôYó?³˜Ç¥ó#Œ?"
æü ?½"¥Xû«?ž®'¾ÍÊ?éÚc¶ˆ½©?¡©ÀnŸ¹ÒOTHER4FGL J1700.4-2746¿î%Ÿßtð@!¼—ú](ÐÀ:C	^M"1À;¸+`ÖÚm@N'·ވ@L'Iñ?Çݏ'¯›?°›»\âÙÿ?æ{—P=Ê?úQÕøÅy?¤; :XÓ?Øß-jä%¿ëàz©"¿ßþè(¿ãƒHõ<X¿àҍÖí·ÿUNASNone?æë'ú\í?Á$2"Œ—(?Yc€N`3?¦ÏVѳ:?ÓPÃLŠÆ?Á÷—ë]u?ê4‰ä3µ?¾ÄsY`eé?'bHé2?î·Íw?Ŋê´ê-?½
"š?ç¶	–¢Ý?¯ïà`óøÅ? ÅcRÞë?"
52óº?Í"(Oeª?­{O‰2?ëÝcX2?™+C¸'4?èǘõ¾?q·¨ÑWv?¼Ú³Y"þ?—xR[ž_?ਫ਼LºKs?ÃÇWàð"ñ?"I"µkð?".}È«ö?Ýh1;P&ù?Ãã+‡¾a?âòö1šÄ?ʄñ¿©r?¡í ƒœñØ?¦€ÞT0`?×Üoèœ?É·µ<Ò8?àåûÒXy?´É©§!Ð1?¯ÿù|±–
?¡iúOÔãù?Ú4	,#Ÿl?³RYÇ¥#C?å÷g%al?­Ô-Þó[{?¥uíSÐ?ÝOþzVÏ?Ñb'7Óßn?­{ø#0¿bAGN4FGL J1700.8-5218¿ïG›qNæ‡Àßþó…õÀ9ØU)þKÀ;uÌ¥_ z@bQãÍo_@ãVg?ÏÚû#L`V?Ïud8#2@â˜E܃#@×;Ëz?ÖÊ¡¤U	r¿ë•X¢žÁ¿çn¿0,¶¿æùÄaÄ@6¿ïþùoÃz¿ÔÓ@h¥ÜUNASNone3FGL J1701.3-5216?ãö¿ôf¶?½¢®â?'ßúUž?'"M"ZW÷?Öò2Ӂ?½S•ºx­?ãR¾ÆFBQ?ÁVÁö¸Œ,?—0ʜG©?"Lå!\?×çuÉÊ}¬?ÀÉçlW¹r?搁Üu?¯q	±ÉU
?¦Í«O;¶ì?"ÉúÙ|<ú?Ñ!*XTf?­ö× ?ä÷iÍ	nÐ?¤Z.åóD?¤ú˜
Ý¡?~ãç*zÁ?Ó-«ÐË?£ß77Þw?Ò¦G›Ü%?½Ëk‰÷÷.?¡_!š Öy?'¯Ýs{1V?å—'F?¿
™¤4?Ò"7›Ud?ÂbÆÁz?¤…R·H[W?¦½3NLnb?妏©Î?Âö §º¢?Úx»"&yM?´AöžìŠ?´ÄŠeŒ0?œqØ
Ì?à+äòˆs?´ƒµÏi¼?Ö¾…l†?«󜤤?°¤Ww?"ïB;»w?âŒ<_'óÉ?«ÛÎûÙ³CMIXED4FGL J1700.8-7304¿Äʍ֏pÀ2jázû]À:ÿȘŠ¥áÀ<w7ð1Uã@VÔ}›6@jÕ`ðà?ß{2{R[Â?à!ï^G3@vn¡žJÙ@[<'¦?ÜëÂFa
?æ÷©OBÇ¿à.Ìț¿çÐÉ{ßto¿åÕN±=û
¿ïæïÝ ,UNASNone?ï½:e#Ê?xŒL½êz?ThühOÛo?P\—/»ë?|HŽGT ?v&zâ %w?ïƒÖš'#??Œðúš¬?mLù‡ZǶ?uùç/& ?‡·õ)b?…›'j"·?ï0ùOÀ:K?‰Cªú•?}øsz¾:¢?}b'"euï?'b¹+ÜÜø?'ÚýÛú?î³dûqØ?|EŸ°­±ý?<ÿ|,åQ?fèãRþ@? âYS(R?x¨;wCÄ?ïs
¿8î?ƒRe¿?j"ýOææ?bºOy"[?Œµjä&)?%èpæøÀ?î¢×I8¿J?¦¸;b…?†ß<½™²?˜‰­­³›? ¼g ‹ì?žÖåKì	 ?î¤~t¥~?""ºÛÈ!?ƒ$¾¼˜ì?'Þiqц? îé	ò?'
$=H5?ìø6ð¬ûÌ?—{ހzúø?….:Û0-?€J‹&¿«?µš¢´¢™?–Ž]}AGN4FGL J1701.3-4924?á¾}9ø°À
2±-4À9Á.^¸<À;=¥."R:@JÀ¾ ·†@ Uûµ¤?ÏÊ,–?Ò,¬{ž†é@:ry\ã?þ<«tp–¿ïþÐW›È?ïý‡ŸñøU¿çÎÇ]øÛ¿å§û'Ü5ö¿ïþ'ö ?â²aFkõUNASNone3FGL J1701.1-4930?ã¯à×†Ã?Å{ï(†Ù?¨˜‰"í?¤ÑË¬¿¦?Ս-½ü<?ħ¸¼Û¤<?Úb)HVµ?ÇW^òÊ?¶'7k¨ÏÕ?²'Aq~6V?ßýHÜxøv?Å'\-…ý¹?ÜÍMDv8?±Ø'Ù>É_?¶à'…Å–?¢Àìíb?Ýz'GÀ³å?±šT´ËÞ?Û&,uyÝ?©Ú™¦…q?ÅY÷òY="?¢$(£>1_?Ú,×i]ç'?¨IuM‹®\?ÕuL÷ï)?ÃbL•Î?µË;¨€E?±Z©mH?â¾áÒøc?Å ž9%?Å4.þSq?ÁÚåÎ?Ws?ÁïB`«D?ÀDD¿o?æ7#â՚?Ɛ?ˊi<¦ñ¾?®%Žž?Á®406?®T‹|Vˆ?äÜ:#Îwƒ?´]îúrm?Ä¡IU"`?£>R1a]#?ÏO%P¶?±?²áubÜï?ãäV‰Ø?³àyÔmMIXED4FGL J1701.9-4625?Á"^¡‰¬À7´·,À9¨3ša?¶À:Ûd53¾s@/©Ì—Á@¥æ¼b~?Ðkj|uœd?àR=à
l@@
?:¬¤8@´™Æ»á¿ÖW}ë=P¿èÏ"Îš¿àôG/iz¿ê2þº…¢¿î?.Ö­ ¿ïSÅ¿½DÅUNASNone3FGL J1702.1-4623?ŦT—JΟ?ºt¼çÐ.?Ïþ1­ª¦?Â\.›9?â–äÍÁá¯?È '¶jO?Ñ)ëdU·?Æ5°;´ç?¶«Ӎõæ?²ls$µ£?䕪\h?Ä7÷6ǁ"?ΗûVD|©?°žB¼yT?¾Àœ4Kª?¥=J(»»?äí£å€€?³;Ñú·€Z?¶Œëv¶3¼?'(³°ú'à?ÅQÂä&í?¤
;h;Ã?çÚ!à‹¬­?¦Õ³×+¢%?¾¨§F³÷?²[øœ…óz?Ðë
OHè|?ÃSÝ,–a?ãµdo…Þ?Ç(㝍ˆÙ?µk;Ê´Ù6?µ"Æ(^g?¾>a`Sc?»t̒Œ¬n?éŠÌZ>Ãh?¿"Õk›žE?¾åÿÏ¿é?¢¸Ý$?¿"\+á?§§¶Âé,?è@"iü??¯[ñ¢­)?''DmŒ-G?xe¬–Ç8V?ÊÏ£Ãác)?°ä"nöÊû?è¸ë;¼?°úíd¥yªOTHER4FGL J1702.0-3721¿æIeqca@+xÚq3À9¦Å¿'Q§À;vy!@ûÝÜ@MÅ2¥?ËbV6mzW?Ð ´«m×t@ZÆ3¡î@ZªBß"»?ï±ï,»J¿´{ƒ"…F¿Û»âï£ç¿ã´U'¿êS±Þ3ý^¿ðUNASNone?Ý/ :CY?ÇÔóªå¤é?¥~'Ô(r?›˜wW:Ԇ?àeûÿ¸?ǵW8(Ã÷?ㅩo÷?Ã<Â.Ÿ`ê?¦"ª'¬?¡áTäË×?Ö3œ¢ž?Á¬\×hÔw?à¨qÊ[®?³…ÂÏ?e=?¶êQb?¢à×é	?Øô‰†ÉTÀ?²~)­ä¯a?ޣ݈dp¡?ª³Ë—?7©?¦ñNq´ž?€Úñ֗^?Þ}ø©Iì?ªß"…~2?Ð@ÙÓµ8?Á˜·í¶?±-{Ò×w?§îñ±†ñ?å¹ã¤æºñ?Âÿ©c;8»?Õ-Éaeÿ?Ç»;ˆtâ?¶5'9"Dr?¸U)Ø£?â¢Ìô?ǚ{–Ï9ä?Ñъ¦¨?°*¨sqÔ¾?ÁØ(ãŽn?¨kº^S?â¡0ñ	?²¢À
¦à?ͧþC3Ó¹?©Uîݹq5?°"áåªí"?"Z="Rez?æƒd2xP?­Ne˃C
MIXED4FGL J1702.3-2525?êÍ®‰s@#à#éêÀ:9êØPÀ<Ğ*"@²Wz>ý?þý@´%?È`hàê*?ÒUûŸž@à•äÙ3
?ùàçß!ä?êý"à¤ðæ¿è¬ÍT¤?ÐCCrE˜¿ÙØŒ'Á¿å³I€C‡¿ðUNASNone3FGL J1702.1-2524?æÓùPRA°?Ëö'[ {å?'e€§+S?z‰xýÖN¾?ÑÄáZgCu?Ì>þdì¶?ãÕeâs?Çš1šó?­š9i½Á?¨›{´—§?Ô¡îÏxp!?Å9DDR•N?ê3àæ›f4?©±¦¬m*?¤pá–<Ö?–9Úä‰ú7?Â/`,‡ê½?¦ aŠ¹ Ù?æÚÚph7?¢:;֓÷£?°Ø`ŠÌz¬?
>P…º?ψdPj.P?¡s "Ú&?â»àä0ì‡?ƾµe…žn?—XØ\˜ŸX?x@Û×è?Ù°±¹ ?Æö!€"v*?Ö¸HjkÈj?É­½	'­?»Ôo¿'·?»¬Ž¥l-?á)MÒ×äê?ÉkÝÁ?â?呤>}#?±€íž{&?°Y+œ9QÈ?êaºk?ÐÆl›‰³È?¯Ø›Í{si?Ý­óðÊzZ?­Hš R0?¸¸ÖÃ?¢•S‡é"V?Ü$Yò²?°+WqàåMIXED4FGL J1702.5-4803?ïO±"®RÀÅS[ǦóÀ9»[>À:曶ªK™@¸HýÏ@Á`Dä5Ÿ?Ý©Ga"mÛ?ǒ&>?÷1Me
 Ò?ûæ6mÐ=¿íöÞï@5?ïõuüŸ¿ê¿Õ£5#οéJ>xᓿå¦ÿéYËM¿ê¶iLUNASNone?ç•Ï+%õ?Å´'ÆÖ,Œ?£"{'Y?¢n˪½?ÌÄupÅe?Ä°âí'?ÞJ¢n÷§?Èr‰_d¿r?¢‹÷€ú?¤<k5ñ
%?ßd{núù?ÆpÎIN¨…?Ø+¿:VØ?²õŸuÛâ/?·\ý•jÖ?£#÷˜?áØ ½å©?²ümPUý?×ÙÌ©U=8?¨~6€ª?±x\!oåŒ?™,%4ÞR2?áä'5#"?ª~©¶ï¬%?âûŽž5W?Ç5ÈӇÀÃ?µÉ'"1à?³¾9/MU?Ԗ~;ð1?Æ{Opom?Ê¥3;ýÃ?Âꬍ"y
?¯™Å£ãŸw?²Ö@˜:bÁ?çzY7~Ç?Ão*1yA,?Îų99?­¨î>j&˜?Àȏ—Hl¼?©á—H×@`?äLª­_–‹?²JS´}¸¢?á-×Ԓ¿?¦¢£˜õl?²­ic­?«h"d¼¼5?èÂݶ
?±R²/‹µ‹MIXED4FGL J1702.7-5655?ê(Ï|ªuŠÀ"u?À	oëÀ8BÃEdŽÀ;EeìÃã@{¯xÓü@ÖÔ=–?¤¶Pð?Òò1ÀíE"@'ÞSó@/;Ÿheš?ïÌ
ÑyÛ¿Øm-_´›~¿å\iànj¿è¨ujhS¿í†ý )Uº¿åxYã¡$¨UNASNone3FGL J1702.8-5656?•ÅnšÎ‰!?¤?âÑR
?ìL'sãÛ?´1r^"T??¸*¹QžB?¯â]lg"T?˜æEÄ°H³?¥j‰Ø"Ä»?è®ã7P2?À¶œ˜ÁFK?Ê'ªhô¶ ?ÀŽE¨€½*?ŏªå=ÔC?¬0iZé?å÷vpÂd?±á$x©`Á?'{U"d¯?¨^²E•"?šh'šß°M?ƒk‰"?ê'àn®ù?¡0§ø
?Âkkò^? Ô'ô‹?¢˜g´Qþ;?·\¿näeû?ë$ż?½ã'—…©^?½'ãêB ?´\†`#M¯?‹´π¸?"Q%ø½4Œ?éâÀî¶ñ2?Ãùœ¬§?ÆñÅ6«?×Íjñ)g?½'£ Ù?¨©ãŽ'E?çG;A¹M?³;BìÑ´o?ÄÚYCNo‹?¬Ùð¶Æ?s*^í¤õ?`ÕÔ°‹k‹?ë¬YØ8À?¢¸˜¤†oŒ?ÀµHZÑv™?¢Œ'Ò=5QPSR4FGL J1703.6-2850¿ïê*
D·@¨E/‡­À:@€#À<8¸®1×@ Àåä@Ó~9Á®?ôæç€,`?؟ND0±y@=®ˆ*Ü@o¬.œ Š¿ï"ôÁ?ïU"âOÀÞ¿ÒU,«¶¨¿åÜ_ag¿ì´¡mM‹¿ïÿû-2h2UNASNone3FGL J1703.6-2850?ßÿ÷z(Õ?ÂÅûd?Ì$9›,@Ñ?ÁCý'´Åf?Ñíë¸AÇÃ?½VîàY,Ó?æËÁ
2>?dzèç×âw?¸àº'ÖÙ?¶—%\A/±?È`ž•ȝ?™Q³""è?àc¤Œ‰2?³ˆ«˜ß/\?ÒÌ2-N±?²C¹#öÊå?Ê^
VS?¬nOúûD–?é_^;K?š'¡jÚzœ?¶¡?Nv:?iÖ|¬'?¾ÿ3Ò?}n?'_))â*?Ӈs•}?À·…iiŒ?ъš†1:"?Ư"g?Úíñ·µ/ï?ÄM!Žp?áPó'mâ?ÍÁpdäR?ÅúäG?ÃGSW&=¾?ÒaŽdáp?É°ù~þÛ?Ù@jœ?·VŒ)0µ[?×[†,Ä?·ÛyµÑó"?ÎÈ–Ì7?±e~$—;?âîx˜
u?©5º'4‡£?ÄÛÔfE?¤ÈòwçÇ?ÏkËÐoç?¤e^¨§µƒMIXED4FGL J1704.8-4030?ïŒßÅß?Û@¬B"£`À8yÓ3[AÀ:LèÁõÙ6@Kû+/@äÍt'y?»¸€®­?Ôñ[!ŽÆ@Œ[J©q~@y2 ?ï֘Þ2и¿Ì,gç𿛿φ\¥óD0¿ä³¼ZŽÂ¿éÚQÎ_¿ïÿÿ" 5•UNASNone?—¨*5p•¸?•ä"kõ"€?Ù2£NVز?Ë!‡­;•‹?â©mò9?Êû¶tyW?²ZƒÛÚ@?²ü€žK?È/³ÞÙ?º±ËŸ?ç¨öBUÔ¸?¿±n·B?¾ZÜý=û0?§î‹N%'?ÛÊë"@ÇÏ?µSm?'u?ܞ],o¹e?´Ñ§N¤X?¨Û‹[²;#?ŠW!Rt¼Ì?ÁS©hw@\?³zȃ?ê\ïðw?¡""Îã³?'ÛÃüà‡?¡SÀÂ3‰?ßÃBݾU?È8Îë,€´?ßãC ƒ?ÈÊ+‡Ã-?™sd¶öù?¢ie(¶ž?ɕºð_Ê?Á#˜¼á ?èÎöå)v?ÁŸõ€l™S?³ð÷ý½?¢'Ö¢x5R?à[CuÔ 1?º?'Þt†?ځ÷—âÆo?¸t#Å*aÀ?N¾ÌPr?v<ÕÔ¡m$?ÅJûØ9M»?«é>¸"b?ê8ÀjÇ?­8vl'…MIXED4FGL J1704.9-4303¿Ñ"Ý ÷S¿ò'U^×%ìÀ9a@®Eù	À:‰q€Ø@ %ù	@Æo@SjZç­#?Õ¥dd®€?꺪ùš‹@2&ù'Ô@í‡@¬n?ïÊ4f?êVžrFny¿ÙÇU¿z(æ¿âuÂú»ó¿îÒ¾©HŽ¿ï¸fC*÷ûUNASNone? ë8X5?3ˆcSpò?P{õB-?'TÎaë?îq1öÈæ?£ºTÃ.q
?¿ŸE*+¢›?¾†x»¹»3?ºÔ1ΌÉ?·u`uØí?豑 èòŒ?Ákrrkà×?Ñ·>Èf·?°èYJÖ\?ÈÂGXL;?¯z"ŽÏ?àóÏ'šù–?³'eéIøJ?°,.Š–—?•»‹ö‡ ?¹z<‡Ë?¤?ÇÅjǎ?êÍ÷÷Ôc?ªŠ8{èë?™sç¶æ?"IET"!ô?–rç',?–ËO´>®?î€ÏÚâþ×?¡!9c2†8?§]ؤüŒ?ªÃ5§Oì?½;DÜuX¿?¿Â>ö­=]?êâ¹Ú=	?ÀNCðDÌ
?ÆýÞDæ±?©µè¨Í?ɼÿdύq?°=p"`Ì?ãÑy®±r˜?²õ•a"¨?˜"—­ÑÌö?ˆÈHÒ®m?»9G¡?¯p
=àß?ëÝ$ Ҕ?°þeø·Ÿ/OTHER4FGL J1705.1-4748?éJ¼‡@À+†±_ˆýÀ9«8bGÀ:ä€üê¡Ê@C"~øX—@+ôË—¦?ÔÏ ´?ØôóT¡@ß	ß3Ø@õkšWÛ?ï{úýŒ³,¿æêÛuÜûï¿äXŸ›fM¿élá8"œ¿åÆ×õõ»¿ïÿÚ
¢ñ1UNASNone?äÜ9àq?ÄOfáq°®?°lvý‹§?°/þG¥?Ò@qÃxU?ÃìÏÃïzï?ߍe&S'?Å×ı"? À%H´°¾? ›€L6ý?ÞZ–0zéx?ÄTÓ	/‡5?ÛÊdbU4»?³¢³¸m‰	?Àæ€oø6?©GnpÏ`?ÛÂ[rÏ*?³@$çvg?ÑìSÞ¬ü«?¤x2>µ€?µ;s'ñ?"ŒÀrjcs?äbt¢FïÜ?¦l4ÿ¸Æ?â7«é[Š?Ãã+ØdÊI?»åÅär¨?¸T͐*Ö?ÔÈ®º¾ƒ?ÃhTt˜Ð"?Èû}êÞÓ?ÁŠÔJÖ¤"?°xÁ¤#"?²Qvè?²?ç²&,S^ç?ÂL††Ü?Ў#@™D¬?­šhÎ*?ćï êÏJ?­'Åwá?â–òwx©×?²tƒ6`!C?´L5Åïó?•F¼BŠ÷?»t¨þâ?¥B§eÐÍ?êäD¯ÿ¯?§Gë|p
MIXED4FGL J1705.2-3850?'þµä™k?õÌ߬£a™À:
E®_ú<À;Ë°Àý‹±@Qlut c?þ(j'TÙ?ÑYF'ÆCq?êøPV×@0šú©]@3D™âê›?îÊâa‰‡Ô¿ÏSJ˜Õy¿ÒZ-òï¡¿ß9çíºƒ¿ïó£¼2?舘TõûšUNASNone?Òr6ÜÇ'?ÃËbáÃ÷?¨Þ'¹¾ŽW?¡›BõŸ´#?å9é:k·?Ä/=Ÿ¸?ÌÐÚΐ?ÈXL)EÀ÷?Ç®¶ʤ?Âuj²Ãí?ã
ÅH™³?ɪȱ³?Þ£'ãª?²y…ng²Y?ÆPL&QÖë?ª×ØdG·«?Ö4ÔZW0á?±à´=èL?Ú³Q©Ép*?­E»€:c?ÊËeÄ÷1?«! ¦²"?×æûu	tü?®bÏ}ã!ü?Åôè$ʘ?¼*6»\?·>RWj<?±h(÷d?ç›4ðc3?Á¡"쏋?·dÃù|s½?¼ðàÊïí?˽ûc83£?ÈMAÎê?æ#è§ô¦0?ɒiØ…v?Õâìôµt?±†ñB'º?̵¼R ?¯Í!Š®*?ܙ?áú†?³"¼F4N?żÄþ"?§ä·™¹k?Ò°Ï>Ò1?¸v"¸'\?á_©/±?¸év££ÈBMIXED4FGL J1705.4-4850?ïÀ¨M€U?ÀÌ}´'mÀ:9V"tnÀ;‹«‹3¥I@8‰ëPÆl@S|~֟´?ÖœÈù¶?æ‡ÁÕÍÒ@ìMìm@8JŸo?å',Rnaݿ∉ÁµA–¿Ú͈ßb%º¿é¹ëžŸÿ¿ð?ïÿÿÊPËUNASNone?ÜdæMk2?ÐÇǹVg/?´t€¶lå¼?¶‹qêbU?ÞÑzì…Nß?ÏwF#Œq?âåcÑ­ÿz?Ç:x}Psò?¥QÄömØ?©€6"‡S=?׊ÿ½ºá?Å\˜–S,è?܉5쩔—?³EÀu…Ñ?ÌïbàJ?©!ÏÌp+m?Ù°RaæhÄ?²ú¡?ã™ð¬/Á?°:ˆaêc?®òlF3Ç×?1ÐviW¡?ÔíÒ<3ž#?®÷d,Ó²??×SJ§t¤?ҏ썲[?¸ýŽìLj?½"na‡"n?á6ªººaÌ?ÑM–[vžB?Ñk¢Oöf?ÆÂ]à'iô?¹ùÂÂ:€7?¼™òևò¹?ä
ö½iF?Èßù:ó?Ò<•k¦[
?±ýLøÃw?ű?ÍTñ?¬¸îW7Ԗ?áueVé==?µžÈý!?Ò-el7Ù?±.÷§¾`Ó?¶š²BÑĀ?¡û;XOÖ?ä&"Æp4?³u™_7#MIXED4FGL J1705.5+2907?ç9Ÿõíò%@AR¤~Ïé¸À:¿5ÜZßJÀ<\m.׃à@ùpâ†@Ðfd¸ç=?Ȓõ%0'?¶V¯d1,ô?èäK8ãv\?þŒ³t·?Ùiå‡ó¿ßsd%Ä`¿êA_f¿ç	OŸz"+¿îìSE!rA¿ïì`Eºõ4UNASNone?îX'¦Êó?¸'w|
?"jC¡²›2?–"ïÁØø¶?¥]D®Ï™'?´
/=ó:&?ïH{rÖs?‹l}U]?yã}s[?y—h©BE?w²]¯µ?'g_èr?î÷ŠB¹Ž?‹¤¯‡7Y?€¨¹É,j?}Ù	–‹®?˜ºZ½{¿?…êÃ&¯/?î›N&Ëé?}ÙÌ¿ô?"M«"J'?spÀ—7?™H™n.:?rÃ>Aá+?í¯áÑZ"æ?²~Óð'Š?ˆ'£ùGhÅ?ŠQ?N#Ãa?®Ý9ìà¾q?¯Æ]ˆK‡v?î
ÓRLÿ?¤â!ˆ T?òÏ-ӌ?"¼5²?§'oPÉ,?Ô&Šƨ?îönJ¥/?—54Ã?‹ñÐ5²?ƒ>6ì¢?¨Ô%Òߪ?"|'äb¥?ìG*OèS?—VHˆ›I¼?¨þ[LBS?¦%u×
?±HѧÅè?ü:êîAGN4FGL J1706.2-4950?å0[ÆÀžÇ†;îÄÀ:ðp@üÀ;ƒ€ýÁa_@§l®)±@‡ãúû÷?ЯIĚ#W?ÞúôþD>@e‰ýDcÝ?ø
t";¿¿å\·ûeg¿ÖóI¨Pí¿ã¾V<"¿ëä ©m¿î÷Æ`!'î?ÞFžJ''UNASNone?ɒåy°´Ø?¼Ì¼Óýºù? ›ãh4i?²–¶T?葈kHùC?ÀŽÓôDœ"?Ý\>Sfž3?Ç0ú"4L'?³*ÓöIX?¯YG|˜?ÝÙ¯w?Äýä3"!Ó?ÙÊ$;sžˆ?²«öB°â]?´Î·+d'˜?œ-¿½Q?àýÛ¹?³BÔÝÇ®Æ?Ùü3©òú€?«"€ÜÕ?Ãl'T6õ?ž#Uc—{ž?ÜMƒ«ñŠò?©µc™jeH?±»pJi%v?¦†O"OÎV? •]¼ø?¡bÓ¹÷?ìƸ 'S¢?®èƒ8c†©?Æ
¤"´Šâ?ÂpXm)y ?ÂBµÀId?Á«³lÔi¤?åì‰âÊï?Ç#¾¡‡?Çì»)·3ˆ?«P흾È?·a—uð¢?¡Zùt.?çžFsú?°Û;¦ŒV?Âw5êPHö?¡£—™@+µ?ʔ Ð3xl?¬j:dš?ä½
P՟H?¯}2ñcOTHER4FGL J1706.4-4609¿àÂk»oáÀ	ÄȼœÓáÀ9¬¡´NÀ:ÜC8cõ@ !¾‡z]@åàdYEì?ÜnÖwpyæ?ÖÝqà˜Æ?ýƒ3ü†Ï?þ±ì<É¿ïô‡'YY8?ïú:þпׅì~à¿äW¬ŸZή¿ê¥cÒ7oÙ¿ÕW`NjUNASNone?Ì(2lAzQ?¿XjöÕ4?²¬Ð›ŠöÄ?¬Ä&ʔð?æ YQÞw£?Â;Çýì:·?ÖqýØ9Æ?ÆhêðN\.?©¿oÀŸp?¦9¯ù'TË?ã+†NÒæ?Ä÷ÐÉ(ú?Ð'A¶ƒµ?°Ô_R]áV?Ã;ì¯(È?«ûðZSZ0?ã!»³c³ó?³îïˆo˜?ÊàóºKk? ³Ô"+gE?´WÙ¢÷zñ?–5Ðj'Ð:?æ¼ÇÝ€ç?£«ÚÂalŠ?Í~"š´¢?µçí:!?µå0úØ?®'ëŸÊ?èz£Ñ;M?½c"‰½ª?¿åQ´¨q?ºãÕ°~Á?±ËQÎ è?²1ê:å½?éÉ뼯¦Õ?½ÿ®¬¸¹?Á?A÷'?¥n?‹¡­?ÅsÃyÅql?¯Ð«èFgþ?æSMÑ*eÀ?²ÉÞ,I?²ÛdÊlæ¬?•¨×̛~À?²•͝÷?¥u֕Õ=)?ëQñÍbº?§Çq_'OTHER4FGL J1706.4-4649c¿'›ãý"5šÀüœü$©-À9Ëû¹IÀ:ôÞW(Ü@=GöŽ½@^ú|2€†?Ö÷Ö»¸þ9?íý«w@	ízÂ=ý'?ÿ¦Tè凿ïÿ¿h`;ª?ïý­àx{<¿éðˆ=ќÀ¿ìZ¬‰`fr¿ì…;=ð?ÊÊ¢{žHUNASNone1?É>X2ú†Í?ÉauÙ÷Ð?±Æ'~¥'?´—‰îo£–?çw™£™fˆ?˘‰=Õ®?ÒdJ_þ 
?ǀL$µ…Í?Ã0-­•Øx?¾
E½^k?âÏe$ê=?ď¼sì¿d?×HZRî?´²)ÞJÏ?ÀeÜ?¦³K©C'>?àTÒò?´íN·ä§?Á¼·éiÞ? ¼Ll"?Öµg¼÷?°Û‰izâ?àŽwˆç^?°™î"	ò#?Â8]|æc)?Á—¬håX?·$wÒ¡,?·x?ël9?è'$Ð?Æ4¾ùzÎ?¸‡¢+{"P?½'G³ý?˸>þÌ?ÆÈnu½-?åþ]ª™àÖ?È'¹i~Û?Ë´©%¹ß?°æmå\?Ä4'¦,ÇV?­·îÒÖ?ä-®+¡ïT?¶®"å¬?ŸGüß]Iç?‡üMÈã?ÜdÒÛ&?»\"Fe·?à÷Ž©fŽ?ºíš•Ô#OTHER4FGL J1706.5-4023c?잏8ÜYL?͒Fiö¦À8…™1"ÎÀ:g°éAx@Xô"&@qœûMê?Ɂ©ù8:¯?ďHy]d@o¿@OÂ@*5³–?ïýFA­¿È+³1fª¿æÅ»Áã¿è(žŸ'×Þ¿ë\½جտïÿúÁҝÇUNASNone8?Äôý~¬•?ÉqvA®?"«ÏØï°?•å¬êŽ?êa$AËí?È×Jðû;†?ÁÊÑÊãi?½gBÍb§s?¦Œ:oÇÌ?£]¾}!ëm?êP‹—½Y?¿˜xzm·ò?È͈`®ê?®<=t?¿]QûÜk?¦åæ·û¤?åàó¨XÏ$?±¦§j¯Ï¦?ÀOŒI?ÿ¢¶C‹€?£=ýFÕ6?ƒJQŸ'Q†?êÇ×ØÕ«? ¼nåÎ?³ü#8<¨?Æ)0 ÀP#?Õ‡b]¸Û?"ƒBv9p¤?ìùÏ]å}7?Æ šzü1?±=R'ƒ?°(`b¿ˆ"?¬ŽÏ2Al?²kå¡ó?ìöÈãwù?¸Ãµ<ôcP?ŕÇèa}É?¬‡Ù*²)?¼)Ïöç—B?¦,Ž{©?çT
­¥?±of†›ì?¥âVŸ8Ú?ÄÅè
7?¥Ü÷õìí?lf"k?íD`Cã?—𷍠gOTHER4FGL J1706.7-5525?â±d0×
mÀ!"½8SLÀ:-únƇÀ;¯2c)›@ÿwšôŽ@°\‰mÒk?îŽ|?@²£?àµë÷öF@î¯?ôÖ@^Ѭ°w­?éՌŸ
FÖ¿äÜ¥R4€:¿ëM£Œa¢²¿è!ìÿ.¥¿ÛBwî¨j¿Öº
›5¦UNASNone?è¯CÇL}?õÜxïÞ?¥­Æ-L™?¥"0ÍÆ?ÊAÑq!Ue?Á†ºTƒ?çÞ¨†5S?Çgó6÷k?—6$?¡ó¦<€"?ÐdMÝ¥Ú?Å|pWŨ…?æTC<g~?°‰弙?³àĵØè°?¢˜¡ÿñG?̾cF±?¬Q ©gÊ?ëNP7¥Þ¡?¤èJ)4zÞ?Je?OH?‡Rø—Î4Î?ÀÒÍ<šv?£"úA£Y#?ã´PrÅU›?Å·îiˆ?»T­<ŸÔ­?·Õnjø?ÑÂ3ËM_ž?Ã`ðTU0£?Þ!èx?ÏêªG*¦?¯ÛÙÀ\CP?·5"ÿ"nµ?Ýãp²ð'´?Í
y
'åÎ?à´Øð<Ç?²\zKÂît?Á;"u Á?ªÅÖdU^?Õø¾·O%ò?°Õ¶ٚÿ?ã~ÒçK±¸?ÂD¾?š._ðÈ­î?¨piÑS9ü?×_t3{Ð?ÁÇqÁì҄AGN4FGL J1706.8-4540¿ê¤B€ÆÀðîÐ,ӞÀ9
:¥"À:x3⅛¶@Òå°@Äú¦#ë˜?Êꡞ÷?ÍWåÐD&@q£EêÅÜ@5,ìG;~?>t3¿è 'w"Œ¿è<yÎ"7b¿ëZÉD'¿äÃ4½ÌÔ¯¿è
q=Yý¢UNASNone?ã]ý%¢…?Ì%öBÖ®?Ãà&=Mà«?É3õ÷y¯Ö?Χ徕C?ȃ½ŠS?Úë)}Á?Ç÷¸U=ìl?ŸŠa==ÀX?¡9Œên$?áŽ7_?Ƴh~)â¹?Ù.bÃ2‰?³-¡L6&'?º4öŽ´…¦?¥2Úê9Á?à"/̐*Ê?²ÍOR[i?Ãgùñ?•9?œŠö'l›#?¨*o†r?‰éÃ5pæw?é¥⻘ê? =0ùÌ?ގϑ"Qº?Ë9k­3e™?ÀYy\%'?À²U\þ³¥?ÙDs¦¯›}?ÎMr·á
û?ÃÜÔdßd?¾Ân؃lå?©–¨Úq?®w(2Q ?ép±"Òþ?¿¯'áÛÁ?Í÷&a,"‡?®ºiŽ]'?Á´®b?ª Ÿ.+?ä;ÉdsF?²fÃðý{
?¡ÚLá0ç;?†ø¿?°^¶¹wöÖ?šQ}\ûm?ìքZ†øò?œÿ…4F~vMIXED4FGL J1706.8+1319¿á®wEB«@=
ù½Æ À::¼µ'•À;ó
÷9ˆ@tŠ‡¿@˒}E¥ü?ÁnÝÃÀÄ?³jzF?À»~ãH@EÝ
$q¿ä#gC8N¿ä>Yl'à¿ì›Cót×B¿èÈΪŸ¿êb!LÖÈ¿ïðCÊZ+ÆUNASNone?ï˜ Ìíó¨?†›e?­'Š?rÐYB?mÀö}fÝV?€÷dÓ¤ºW?'€²½¸û?ï»c•"z?ƒÊo÷g?\>ÚêõgX?mŽ¡Å?kL?{>~¨kj?{\;¥R¡l?íš wIJ¢? úù¦Œ¬?'ã(øªrÆ?ì*S?­ld	j{?š÷辡º?ï":|ö?kWÄÙT˜?fm£ÑfÊ?Ny±´ëG?…¶`ւο?ge¸lö©ç?îå""ûò?š,[){·?Ž.UiC.Œ?‰…Ì2H&µ?"Hbȶ¸o?'ݾ"Eë?ï=º‡ó k?˜…œNº)/?mQdú¤û?~×ýN–"?"ž}U¬Š?"ÓI=¶™Û?êô%Ëì?ª÷w`ص?¦î¬†áO?œKmfŒ?¼ç€Üx*M?¤Ìµ'ºü?î°ø…žv?Š÷K¯Ÿ>?ƒê>!]?sñ5™‹H? ë¨MÅ?†µh˜tõXAGN4FGL J1707.6-5351¿å<–¨ðÆôÀßþmXÈïÀ:dT§!A™À;ÁåN£Ò@—›±vÚþ@œ zûI?ƀ"9»¸}?ŠéÖë+)?ÈæX%?èhkêòÃ?ï´Ó³¬j¿ãSæ1!àû¿ê.‹-Æ¿ä㮀†x*¿àÒ1@ìF¿Ü¥Ûüëx‰UNASNone?çˆÜP+<?Ézš†î5?|e1Óü²¿?}òJ3ϖ?Ð|²—†2Î?É0R¶¹ÃŽ?ã¬m…$Ó°?ÅKqXez?Œ~%¡"‡?'JÉìŒt‡?×Ã3Èü«?Ä¿™J5Д?è}å¹dÌ?¯e§3<Ñ?'ŸO`òPm?†(tN—¤?Ë´š|öÿ?®a›Lø?åwjkiì"?¥›Nv?ŸY	(…
?.wiõcX?Óš'LF?¤¤íbS
A?âG;b€?Ê$ðM8µ?Šü*¢.ØI?†"Ê*<0á?ڙ¨z)‰3?Ê pr{??Óï‰V;²?Æ{Šì=ç}?—|‰
fb8?£‡$åÒ'6?åLW	b?Æ\h¿9ÄÐ?âv™m"?´½Ó]Ï? Ó6—qh?'þ·Ùà,?Ùά	w'Ì?´R¤æÊg?×ZŸ¢‹õ?­áƒøyw0?­ŠƄ©à?–•{¹
­?➱sªò‡?®ÖbŽҝMIXED4FGL J1708.2+5519¿²ˆãÙå¬E@BE"V!uÀ:ò¼~ ïÏÀ<‰
ä¹S@4,AQ"@ÁÛsX½?Á~$É
$¬¿²¿^z3͸?ðÞu†"Ú@•^XûIJ?ìñeh9¥=¿êŽÆÚ
M¿éóëÇkd¿â³@S'D¿ïÿï¤h)µ?ïÿyYˆUNASNone?ï×Øa*'P?rÜû,'nŽ?iÜ%ßPp¥?g»šÖª?\–ñôy
?jÃ{8ß0Y?ïgtPŸ*?'ÃF˜'g?sƤ÷{?îgë6p[?Œ?¨˜'EÕ?Š(DûY=Ž?ï@üÿ3?"`—".ÄW?s–÷5¨™Â?tZQêŠK>?"Ò.ªp(?JÖÛ"?ïÁ˜fÇ<ô?aÐÜ·µ"<?dì&¦RO±?Qwc'M±?t½¹h$Ú;?Y+v
híV?ï§_4:f¦?"Zª1øŽ²?'Wì'q?ƒ(F×; ú?\Æ×Ñsáµ?\Ҕg«?£MŽ?£¯5?®À?€+õ"¨¬O?‹¬/`zE?¡údëv?žéê2ñìW?hï¾Ð?'¥²¢ABq?€÷3ÍÔ?yéí'ñ¾?£[¡%$?x'ûÚEJ?îõ'áqþ?ˆµ?gt†?‡íMÁ}.?{Çh[Ìk?•W"93¬?
€Ë=‹AGN4FGL J1708.8-0923?ë0rÛâ@1Îû"‰µÀ9éÓbCÏÀ;tgVPn­@¨¯Ýþ£_@Æç£è`?ÏêéWòÛ)?ÎÀ|œÞ…@úälü'?ý¢™gŌ?ï;š«'"?ë†'_8u¿æ3ý}Ħä¿è:¥Ž¦¿ïü‰Þ™–¿ïÿþBe«+UNASNone3FGL J1709.4-0917?êp:ùXσ?¸"-	§?šóþý¼ýÏ?¯èÉ<²?Âà";ü?³Ü¤ÝI¼?çC5"»[?Å
Üî¿!$?Çnµh4ÐJ?Á+pFl©?¸ˆ{‰ð '?²<
Òo‡?åzëLOõó?±$¿ŒyI?³jq¥ï?ŸÜêbpÛ?ÐFŽÊˆ¤Õ?®\ŸÂ}"?à•ÁÑO?¨gÂg…Û?ȅë;ø©Ÿ?¤¢áãQ¡ó?Òºá6€"?¥ýÛ¯&?ã)Æ
ú?Ááþðý~?´êhڃ?°Y¾–?Ô­­Ù}Æf?ÀòdEÈs?à)×ݑ?ÊÛÏòϞl?ÕÈÁ€Ï"s?ÊjÛ@-?ÃÊ´Û¿Y?¸Õ"Èð3?ßÆõ|à?³àë-Y+?Àûðnñ?§ÛNÝ1?×»ìӆ?±*m‹bŽ?ÓkX͐Zð?®!v8Ý?Ð+ÿÍ£?³°õ°åžQ?܉|o×m?³?±·Œ©MIXED4FGL J1709.4-2127¿ÇZ\Þ¹o‰@%ãU>S"À;8ÿI÷š×À<ǂ4"F|@ ÝɅ¯Ô?ûT^[Õé¬?׆ncàÐ?ïò%ÀoF@ُ>Õ(?üïTa+>¿ï2QÁ"³§?ïýµ7"Ñ‹¿Ørê"ž ?Úu^<¿íAWîÔ^'¿ïýÜÚa
UNASNone?âÐ=Í…?ÃçL,åñ?˅áXŽÚ?½Å
˜¸õ?É9's·\Î?ºÕ2-ñø"?Ób6Ìôs?δˆA¾¢?àª3I??ÐP1´`¢á?Ɠš§ê?ÂtÃ1©¬?âr(Iˌ?³'Ëù¸õ?ÎÐÚì}ʺ?°ÊØ	‡a?Çf"â[?¬ôW(?ÜT¤òé?»þ%N2ó?ÜP˜•ð?Àœ³ÕZ?¾PK]?¦x[¶~ ?à]Ö¯ú"?ÃÌ
ovÛ?г~ÄÎs
?ÀQsDñ ¿?Í!§¶y	'?½m‰N?K?ÆÇ÷4OF?Ê¿l9?䑠ïqÆ?Н=÷÷Ô?ÆñˆÆ(%?ÄJGÎî¦?Ýúj‡æÇR?·L°ºþE?ÒxÑêæ4Ê?µø±?ô#ã?χfÇ?³ï8¬u½'?Éõ'p¦?¼á¼ïñ·?äQž³jV?È£¨ÓÀ©J?Å­Ž??ºÇìÆÅÕ?MIXED4FGL J1709.4-0328?ļ\Û±}@4ÅE¥ü~kÀ9hAK#êÁÀ;µ´+W€@˜XpÚ^@ORƒZ'ô?ºÛÅc!?¼…ùԗÇ\@tt–ªÑÐ@ÌûÎÂñ,?ïʑô‰ª8¿æÃ:aû›¿ä	z!Úh¿æFÔ©¿êIßÇü.¿ïÿ (ÿӊUNASNone3FGL J1709.5-0335?î&¢Žz?œ-êSX]2?‰z~ò†ü?{¬ê<[?§7†s«?™0Å«×oú?ìˆÁ£?µXŸ½ðÇñ?­üàôs›2?±v`+?©w
[S*?Ÿž1ÙÁÒÉ?ëeÒ9É$w?¥ïÜ"Á?¨">hø?š¡¤J 4?¸‡NýìÈ?¡´ZŽaš?ê1ÿ÷œ"0?•Sy˜«»?°öϼ¬žM?‡mò†K²Q?½y0‡K'5?ŽÛÞñ9)?êÒªrb{©?²}lÛÈ*?¦Wê\0«º?˜z)W`eÑ?¾>·=÷åÞ?°‰ï‹u?èDåD4YÆ?Á©÷þ½á?À¨ÓÖ"Ù@?½)öø´ ?¼‡.2N?°™@\
å?çâ2"ý¨?¯ ­Þ?Óå?¶¡é3à­)?¤(÷ÙvZ?Å&A8?¨½Ü7+˜é?ãz9B'?¤'ücµ©g?Ã	׫^NP?òæÛÏp¬?Ï
CL'mO? ÕÝ]6é€AGN4FGL J1709.9-0900?ïíiÑfÖ@1ÆüvÀ9þCiâÀ;­iQ;@z*¨J6…@Æpº}>ð?Êpkø̄þ?âžÏ™/çN@œ4;pïV@ìÞDïHM?ïö8 WäC¿â @|ÇÑ»¿âºJÿ'¬˜¿éUao0º¿î×nF.¸z¿ïÿýç!éUNASNone?äá]°ŠKô?ÅË[2«£Ý?Ї¹Úy*0?ÄINÀ#éa?¶Ö+5B¦?±½ð—ÖkŸ?ÙÅæ³A¥+?Ìó=W¡R?Þ ؛?À?ÌAR…³Þ"?À[ðèF6+?¸~Ehqh?ÛuNQ­ØÒ?³b7uR¶ˆ?ÓNæP	5f?²~úÜՃ€?Ñ;Ë^HñÈ?¯¥Ê?ÓóÆ$«Ê¸?¥-`°?Úiðxg^£?ª8"€9tŒ?Ñ¢IbìÖ¥?¨AɝõB?ÚÀ—‡$è?Ä¥dÉ-[?Û¬|'1Qm?ƽÌý|ˋ?Ã%×ÏyV?·wN…?È4^·ˆí?ÆÈÌ·m?åoh8.q?Ë»7A=j¢?Âfà½M?»«g6ð×ï?Òþw'1zÕ?²
&"l-?Ù2ÉÁTž"?¶þîÆ?Óοyæ˜?²|6^ƒ:?´Áš(ȑ£?"<ïÊ}½?â¶âf€×E?²ñŒ×ù­?ÕaÔ¨°°.?±ò…«~ˆMIXED4FGL J1710.0+4629¿ïínýR•h@B/Øf€À;	|gY«mÀ<¿¹üæp@±Æáü4?ü=''N#z?׬9¯N?ÚÚÙjj&@?mƒ'˜?÷Ï'EZ?¿C¬ÁÙB–¿è¸V¿×-۝ôr¿Ý"§BÔ¿èY`Y+"¿ïø"PŒàNUNASNone3FGL J1709.9+4624?í¿[_¢'?ą
ÄÜ?'m%'ù§?¦MÊB–Ãõ?¯ˆîºS¬?ÃօՎߤ?í©^oïHš?¬jô‰õÐ? \ê;ȃ?¡'ŠÆ0ë?¥
.ÄgN?¢x›ªQ3?íûf-0À?ž;¡Xå%?'Æ­bŸ?èvg¤t?¦æFz˓¶?—ó"ŒÄ†ô?êDtðܐS?šþbâq{x?­¤<‡[?VÀ̦pÉ?¿PU©î¶?"Ú¬*ã$õ?íÿÐJ/Îû?±ë[§ÜØ?‹Ðè'€©?´å•ê5?©=Ç e{/?°ûŽ7X	k?éޜͣñ?¿Ÿ/E<ö?µÄ	Iá½£?¶æq§vÌÇ?»GJPQ?± 2hߜÆ?ìé	Ã'n"?¢sàÓh?˜Ö/E%?'"pÖzâ?²—¼Xb!?ž[ùÃ(rá?ä0¢è«X<?­]fÐ[²?´U~'…å?£T¼ê?҉v?§Ð?ªñ*DåÕAGN4FGL J1710.1-4541¿îöÏsù«À·'Ôà˜À9Òí˜oWÀ:Ä]ºÆ:@ ÝÒÕzp_@­D¦">?ÅáÈÇÚt«¿öå=öŸ?ß$¥Ñ¶A?ûǕ*t¿èI ]?é|×V"ŠŒ¿µIÖã§å¿é=êFZWd¿å<jIIõí¿Û+Í
dl'UNASNone?¼"ù˜÷w	?¸Ýø¡Ww7?tvω?v¾xŠô?ìR²ï£]à?¹ •-Ƅ+?Þº–0zéx?È瞉Ý(?"X'œ(Ê?"­"H»kã?à,c…áUñ?ÈIh(ÞE›?Ózy¼70÷?²_…`L?¯*ûÜMÖõ?Ÿrª—mÅU?äPdrµ?²ÏTÑ{xÀ?Íh"HÌÍy?¨bâa)RÄ? c²2ëÛ?w+q	
øM?è1Y_}Ò?¨©>éyõ?¸¥YÒjº?¶ÇªÙ²äC?Øÿ"áµ?€iBµNÊ?쫤¡¾í?·´ÖU†O?Ëÿslx$?ÂxÌS™ôÍ?,¤-.Qñ?˜õ)ù^â?èƒp"V}?‹ühs?ÇÎyCҁ†?¨ý=57?¬ÚT'ŠÊ¤?žÙ·ýîéé?è>¼f«¹4?­rS`x†g?·OIE5? iió[#_?ÙëFŒï?"PˆøM`?언*uÁÅ?¡z÷‰b4–OTHER4FGL J1710.3-3039¿èÛ£•NŽâ@¯¸á]}ŠÀ9íŒa¢²GÀ;"\sž]N@Ž`¹~;o@Ž8¿,Ñ?Î=ÄfKä?Õ]mÄS¬z@˜:ôȔ@0…·e¿·òÅYç?å«ö"o³í?…§	Þiñû¿á¸FB"‰è¿é¶É™"{¿ïò…Ãù¿tUNASNone?ÇWÈm0sÕ?µáÿ+?˜óVŒ=`?uðG%X?ébu*þ?¶
îµ±¦v?×–,ã¿?Á4çX5Ã?¿;Ö]Lë?²{í3M?à'Ñ.ídƒ?¿œÅ+\"?ÜŸÆ.x?²•Åtð²?¸«•š‹
?¢§£ãî~-?ÝÈzÓ/èP?²Ï«C»À?ÛÜÚîÅèN?£åJ©
ÙF?½:¸£)f?•Që6ñä?ÜÔvèrMX?£Ýæº.›'?²iXƒ˜´?¡Œ—!?©êÓÔ%? ú('Í?ì'²K—-?©¬}{D³¨?Ã×ajÔ?¶Abù.S?Æ+C¶Ê=7?¾.þ‡ "?åV·Ç¬ý?ÁK«Ô?Π6›xs?¯Wñ¡¡¢?Á7£õ
?¨O8rC[£?ä¤pÉQÿ?²ŒÔ
@?ÌGgí*?¢á6ÿ/?Â*RRÌð?¥Z\ÒDÚ?ähp&Œ9?«Eê,õ{OTHER4FGL J1710.8+1135?åý(8·	@;‡dº"¼À:²?d™ÝŒÀ<*.wÐ@p›ž‹@}ãZ­Ë?Ù´…-Pñ?ïÿþˆ0»Š@¾¼@ŽÉ@ÇÀv?ïíöé	:¿Üè@Ü;Ç¿îÓä¿ïÿÀ¿ù)Í?ïûJî:Ü¿ïþ@ý÷DUNASNone?í¨®¢•@Ä?ºmüTFJ´? ô
ÐÔÉ?®ˆÜáV—r?¥]!ËÛð?³¯sß®xd?îìq­ÂF?°Â¬Ï¸a?•‡òcpxõ?¥(
HùÜ	?šzkþ¨R?¡[L0ބ?êêÔ­Ÿh™?©öLà
?±èÏõ'¶"?¢xz܇Xc?¶ÀŠàø"?¢_jO¨T‹?ïEÑ	ê±Ü?ˆ¸*ÕöÔú?mÚµ~3°?qc	v™?"ŠˆÚw?…Sªnuuð?ìש*
ù?½JCX€†?²µ¾ÊGæ?¸ÑÛõ÷¢ë?œ¨½ðS?¨¸ü}—ïñ?맋æŽÐú?ĐBžÇ<%?²BÇ÷a1/?À—ÿ©³?°€ØÕr!€?±)ž¿0H?éj;L²?«üö𓤮?µö€êêý·?¤1ò€
ˆa?¾¸¾´ƒ¶?¥ëçÝ?ëÌpF,>?¶p(³D¾à?žÊhISb?§"KgU¦Z?¹éãÍ´8?±1bw¿5RAGN4FGL J1711.0-3002¿ïÜٕ©@'Õü3ÃÀ9ç…w£¥ŒÀ<ìxc¾ì@äQ&@áf?È9ÜÛÖ}?ï@r¶ÖÁ@Å?9ѳ?ðSœà ?ïÿÿ)@k*¿â pÎI¿Ñœž|ƒ8¿êYÇòrxÿïü"Åý¥³¿ïÛÖ¿•UNASNone?Ýaú§ï?¡TwÔâjÐ?á]"CªŠê?бC²?Ü7b8É?Њå7bþä?Š ^T«?˜£Æ
"B=?é…d-|?Ãö2GŒà?Éè i›¾Ò?ÃÂ,ñáÀ?ÂÑÜÝ|Ñ?ª|è/Ö·?âmÑ	‰N?³ŒlòÊ÷Û?Ñ»oêk»?±1=¾?k
]¬yŠK?R&ú/¡M?í¨˜Áñ/?˜•Â=Šv§?±âìT«t?˜='h­M?Žä}I€?¡êd•ßX?áÓb2z%¶?Î}'ÙG?Á?ÛhŒvE"?ÎÏ=·¾?'Æßëw?šÎI`á?èru
¦ºG?ÉúÈ£v?Í	½Ì‡`:?ÉT¹±£6â?¸gyœ0Ý?¤X}Ç5q?ä
iê™*M?µ6Ún·Gô?ÑÑMÊâO?³ös&wÀ?>kî
Ðø?0FŽ;Gˆu?î4Øp*Eµ?šï€"½m?¬v`#i,8?šÔv_8çÖPSR4FGL J1711.4-2526?ꢖ.oË@ ‹ææS†À9¾çBsBÀ;€¨AÓ	'@ž†¦!è2@©õ1?ȇiÁ9Æ ?Ìmš7NJç@MNûÖ7@ºJyJï'?ïì2ðî¿é¨/"BAÄ¿ã%DȆìï¿çÝî'ð2-¿ïÿ÷fÔJp?ïÿ!ž5_³UNASNone?Þ`óH?<‰?Â×a)ªb.?nÚ¢O*?•8Ñò÷,?ßÈ
·Mµ?Ã&ó~\?è!è&^R`?Ã+_8cˆ?¢%—IuNh? ¢S°úX?Êîù"ÎP'?ÁD,mÊ?恤Çcñ?®aX꺺?­ô¼ˆ?š]ËV	Š?γï³N?ªÂŽüÏÍG?éóÒ;1ëq?£Ùhã)–¸? àQҚ?~ÞB2X˜?ț|i?¢I¬ù÷?Ê8/dz0¦?º£gΛY?­2ñ¿¬p?¦¨'àáºl?çžÅ
"66?¾¦v:«?ßKƞE·?Í%WþC½D?³è˜v­&+?´d1-aœ"?ÛºD³ìµ?ˌPc&Z?ßsÒhJË?²f¬}+b?º¾¬-U?£J¥n"Ã0?Ú6á'©à?±iÀ'³Ÿ ?â—OxŸ_?´ـ$؛?® ·qÑš?"óM¾²?Ø0ºr'(?³_búSÌ9MIXED4FGL J1711.9-1922¿èsf*Æ@'PoiDg8À:]^ˆK"|À<eˆEßÞ@g¥3€µó?þÆxõ?Æ6Ükü(?à{:Ôd¬@Ê~=ó?ütá0‡o?îß»‡*+M?î!ÆßM¿Ç?œ7®˜¿à}€(¯K³¿ìÁ=ÐE'¿ïÿßHÐSjUNASNone?ʙÎtäûº?¹¼>ñ=«˜?äCç‹j?ÃŽÐ#)·?Å]!ìí\B?·ié,ük?¹ÞÇOy(Ð?µó³ü>B?çî=AÌJ"?À¹³ÍCâz?ÃW§NìÎ?»Œ+îùÑ?Êä,~§ê"?®¨é>ƒ¯‰?äýš—g݁?³·Rç2É?Á%i#¸Ÿw?§ïŒÏ¸Ž?Ò«d&ú?¦j¬êUà?á.ñä«´?®D÷°6z?Åî0Ñ=? «E×/?ºÚ|ìBf‹?¬•¥HmdÚ?æôÕJ?Áƒæ8•Ò?Æ¿sÛw"?»0¿1ûò÷?­b—›v£?°éͨX½ö?éòÁtŠ?ÄGBrºÌ?ē8=o?Áwóþ%E›?¾²6"²"?¨Þ–	''6?èe@Ú÷Ä?´­cú&±?¾ÊFñ½-Y?ªÙUte?ÀôÈo׫?¢6pïCg?ä|è#üo¹?µj·§øo?Í—72q?¯ˆ%,B%PSR4FGL J1712.9-4105?ê8Oä]¦é¿ò—7¿‰î+À:NM6êwØÀ;qäõ8@#Áåh$,?ý"B
y?Æȶè‰ì¨¿+L€ûµ?½YVˆwÞ3@cho«­?Ô´­Vœ¿ïùͶט?ïùÞHS'?³LyKµ¿ï€Ê`"?ê"ÄÀŽÐéUNASNone?Ô0(V¶E!?Ƙ¼$?bz—N§_*?\àL'L;?åÕq=Üy?Æ0^†aó?Òwت·µJ?Ñ+‡"· ?†+,yÞ?{+¼¾¯?ækfúF=ã?Ðý¼éÕÇ?ધÑô1ž?²‡$†æò:?£të>›ÔÚ?—TöùÝVQ?Ü<óÖ.©?²u˜ÕXÊb?äÈ'¡?³Ïݬc¸Ç?~—=u3º>?sƒ¹X´Ëœ?ւæeë?³´ÜëÍ¼?Éâ&+Éî‡?Á™
¤ûš?s£ÙZBn?qÊ^C¾Vù?é`.œXw?Á*ŠUŒ'
?Ð?ÑɃ9?Ìþ29Qõ?|2íÞ­Yq?'­¶ã՝™?çÃz;þ9?Ëã	 ÎÓH?Ö`ß+§¬5?²É
Ðõm®?«¬(S»{Ý?n@3»ˆ?ãÍäÇ6Ø?²ê¾z¼™*?بšù"Ö?ºÜ]ùÛMÄ?'èðGdé?'`bnɲ?ã5óŽÏÞr?»MÜèßäMIXED4FGL J1713.0-0521¿ìB@ƒeŒ@3	Ò9XÀ9±ZI!²À;Š$_ZÙj@_µ֟	@/«|,Ò?ˋ"ˆk?Ҝ"$'\@ob@ÛBà™Þ¿ßÞßHûG¿å¾»öº²¿ëò¢IkƒÝ¿åÈ7½±¿ïóˆ'	?íðh]a…UNASNone?îøT^•ÑR?Ÿ$¾‡VúL?íø™>ââ?‡ØÌÉí€?˜ùöÊ"?—ŒÈgò´f?î~ä>$ö&?¨>DY,^[?•zqçˆl?ŸŒ">—‹?š©tÐXêÊ?˜¢˜;¯2?ëRáç?¨
Y'•ã?¤6mwÃ)7?˜ƒô|û9ƒ?»MºW´ƒ?¤7¨˜ƒ?íÅßÿ{î?'˜ÓÝŽ?‰GTÃÊÇ?n×îrõ¥
?­m°(C™q?µQ[s›?í\ý6¡þ?°íÛ¶m¼{?WxO?¡â=!s˜(?«v"l?5£?¨Û
·‹‹?ëʌ1ÀÜ?ÀI(ˆ4ln?¯Ç‰'¡"õ?·¥"Áª¶¡?±ÇÙ§ÌnJ?®ÿèïG?ç	ѳø{¸?±Å›m«Àh?´Œè$+h?¢–d@RrÂ?ɒE"°l?­ý:줩N?èœÞL?°¡Zr<U?¦OS߬ø?'ÄL&nR?ȱî'²«?®§Qu
›AGN4FGL J1713.0-4236c?êxßÚh
RÀˆãƒÈvýÀ9t«ášº+À:Î	ԕ+@ Q(;³_@såÍNÓ?ÏÔ߀Xªç?Ïo¹vXÌË@ía¥6…Î?ýZ
…#ÀÏ?ï:`Nq¿ávŸLa¿ÜI@¢B¶¿ãy[k`¡+¿éÊìW¬@¿ïóGŠÙvUNASNone ?Í­	Ò«w×?¼iÊDÃdª?±!˜'D?¤Ñ+LÒ'?æt§"Â?¿Ãõ'ZA?ÓhXŠkåh?Æ%ï"^-?§\ŽXñ?£y$NÖâ+?äÖ
Â7Ý?ÅN({Žª?Ô­›je`?²»êÏ|?» ù™Å?¤–ñ	ø9S?â~u'z?³b»É?ÁçgÐN?˜UQT×(ã?¸-]ƒ¯Eª?•úe_¡?è€z[»½†? 3pQ?ÀãîkFå?°{Ž]'°¶?³q´1Ò3_?©ì–ÆÊb?é~}^{?·ƒ#Ü¸?»sø	ç_u?µÓ.[ã¬?¯ÓÔØþÂ?¯²aáxSÄ?ê"C°ü.1?¹Î?±¤Zñ?ÅiF†ˆV?¦á-ñ™¤›?¼xj	‰¾?¤Ã´pñ•ë?硶8%?®Ð×V:4´?¤ÔJì±'?‡2L–L+S?»O£V[×A?¡ãõ%Y?ëHÆæ-ñÖ?¢¤Œ¨ú†OTHER4FGL J1714.6+3228?à[ídz†Œ@@ÆÂT£ÆÀ;ª{jÚinÀ<äŽ^Òô.@!õè?û³5L'?Ñõ£KÛ¡?²º·¡lvÌ?ã'3¡m"˜@O?w9Gt¿ï îzÔ]?ïò®Þ¥<e¿Õ'*g2¿ïá.žxük?ï–kFŸ÷'¿Ü¾ïÿ×¼UNASNone?ïâXc)¬2?fNúœaz?)Þò¨ˆï=?+{'mHÛ?l	­ìˆD?e£"øú\?ï ¨.æP	?›Õ@lE'?VÌ6B:ñÆ?r9´g2a¥?"ümu叅?˜¢yžݱ?¯EÓI?"ÕAAg4?Gs­Q?…DnNO3é?¡,b¿ªßÄ?'ºú¥=µÅ?ïܨc@9?a@7¦Ö??_Ñ2˜"ë?UjÇ?qbOF&J?a1æ-!E}?ï̒Y«ºP?toәô'?<x.§Ü	'??Oé£}J?wïP:là?s¸tCÕ]?ïJ'‰³P-?¤‹£Ù*ׄ?a!qò8$µ?‡F:u¬?"‰ ŠöÿÖ?¢ÔDÞÓÌ?íöÊp7[È?™£óê¼ÚŽ?"w	¥.óê?‰'æ¢+¦†?«u–"¬z?–%ÔÞ^ô?ït$<uQ;?…û4^˜{?* ÷©^ô¨?5Ë)%r%?'F6zx\¬?…ñ×ùD²´AGN4FGL J1714.8-1421¿ã_û>éäz@+·+ˆDÀÀ:™âàíÀ<Fƒ
â@Rzé*?úË$£Mx?׈†KÞû£?áÂZ£Š´@E܃#6@AmÙ!næ¿ï""Ÿ´»´?ïýuÁÎ#¿ÚñÞ"Š™¿ÕÝÏßäØ¿ås‡ìÈ뗿ïý
a½_GUNASNone?îƒkgW'.?,‹Ül0?{ñ¨(ÑH?s=­ÑDŽ?¤Klî?šéßäú¦?íï÷ÅQ‹ì?«§ Ñð}?"A‹"`?–" ÷ÌsÄ?¦ß½á¿¦ˆ?¥˜5m)Œ?ìd¢wÊÎ?¦°ÓHÇ? $ìA³ÞÒ?"Ìr8ƒ_?´Èv"‡n"?¡áRœ®A´?è¨à·˜æŸ? RÕ4ÜGí?¢üdA%Ã?"("Fj.ß?ȝ|Gy;U? \ô×ÃX?ì²J2±¶¤?«æeLœ!?–š¾*õ+y?'Èäÿ'?´Æþà"ó~?¨§Ã`¹êw?êáŸÓM"%?½VôWî?©•B¸Z{¬?¬9O!¾P9?¼(`
E—þ?¸B)ê5ô?éhƒÞ,¬Â?°,)P´·þ?¨±
B†à?›ð¥QÛ*c?Ä]"F…¼?«ž;ãݔÙ?ãiÑ}¿&$?¯"²,n/?¦T6#'°?•ùގýE?ÖaÖ@¶Jø?°GžãÑ
^AGN4FGL J1714.8-3849¿ì"üÛ¢…¿ÀéÕÖX½À8@NÕP)
À9Ì:䜸@—áŸ@2êRï'?Áùh6J>è?͉—Bý*¹@Û%ö3Îd?úX»¾¶S?ï¯Ö燿åÌÞý';¿àKeè'%¿åìŒñª²¿ìV/n¿ìêßBEJUNASNone?žuã¥äþ?¢¤ÔjÙ?ÂM8ú¿Æ¡?¼n+	w?êy¤iˆ?¿v‡}¯¥—?ž*%'Z]?§Çñ…c¸©?¾ï/š™Á)?´ñP¡1É?ë0Èà.(‡?·¦Q™E?²Fð–åÓ?Ÿ-En°H?ʓЛ¨+r?¯Ñ¡wÛ?ç-Æ{"¹?±¦úíPã¹?vû'‹R?\ŽN/¸}S?³F™ÿ[o†?"Ç/À?íjöÉJŒ@?"ž±Î)?‰÷T«kÅ? ²ˆì·É'?ÄmŠ"et›?»¾^䫪'?ê|ÀË'?½mW(RPý?@e·%N?˜A¬cCóÕ?À«´8×7	?¹Â'RølÛ?ëXZà9?ºÿ
À+?«ˆÍ\~Uý?™©J™ñ?͛óÏM¹$?³J>™Ún?æàv6Víç?´âiÎ(?Sûg|'y/?C#ç&åÞ?¸"¤nG?ŸX*¡???ìñ­ÊSã?Ÿ~LäOTHER4FGL J1714.9-3324?ævq€ÇÞ@ö¥
k#À9oNäHÀ;*¯ÿ6¬d@ÅÛêÌçû@òzÞÃo?Țk%½Ô·?Û}¶Äͤä@5" ¼8?óH}ˆkI?ÚZÀÀÏéb¿ßð½Âôu¿ÜZе
¿ä3ò«ƒ¦é¿ìl¸?wT¿ïþ'¼ÞB@UNASNone3FGL J1714.6-3327?ŸKYW5"?•nqiþ
,?Õ¹þñY–l?Çàûšü?ä(¥»tá?Ç×Å!:jé?ºðš©ûù?¾Ã(\ÅÔ?Ùâ'í¯ÆW?Æ}"'-c³?ßa±Œeº«?Åây/IwK?ÁªT¥|Y?¥ÆÌ=ôÈ?Ö–Û×µ<?³¯mH0Z?à"±¼êÆL?´ó=x&D?±'*£Fà?‹·µÍý…o?ÐÞüùÿú?¦F¡¹ž}Ì?åk']'^Œ?©¯Ò2jÊõ?é˜©gi‡?U<¹"`?Ьuqú¡Ð?Å?(ܶ?ç2äOS?ÅU–ë‰Ë?ž×P±?ª³Ø&ËH?Û¾áß-¢?ÍÝó÷Å/?á*=T/"R?Ìd¾T '?´ Ûd6­³?$M%‡?ÔÓzj\ô?·±ß'(?ã^VCûÐ?·‡Q»Cy?–¨Ñô=¤Ý?{5On…uG?Ч·!g7?°<Cœ‡Á?æöÝßf#î?°ÿblÏOTHER4FGL J1715.7-4239?î_ð;ÍóÀðCRe(À9ì) ã9÷À;­e(xÅ@¸dC¡j@õÆÛò¾?ЂV¼¥7]?°	ž¡l2?èk¤Éx"v@ٍ\õNv¿Ûàÿß"?ï¸x·¡Â]¿è3¤Ýšzj¿ëU—Ià?yë‰%ƒU¿ïÍõ´L£UNASNone?ÕWEY®û‰?Ç"ôî÷;ƒ?siZ?pšöò"ç?å.;&Ǖ?Ç5ŸqþR´?ää|hRÇ?È¿7G??yO/_ãn?"«é¹}ËÄ?ÕÑ}ÊõËã?È=ïŠøþ?ߪ‡C'áP?³¸ï¾´ô#?©'+Kˆ>¨?šòW2ÝF?Ý#SS†‡;?³#u˜6é?éGt¯â?¦T'ÿ¹™?p¯ecª?al
a•ÛÅ?Ê\´i‡5Ç?¦(sv A	?ÐI¹~ß?‰†Ô‡?|Yړ<8è?{ªš@[+t?çĽ&fœ?ºQPÍS?ÚÔZ7Äy?ÉÆ÷|è?€­ó}j
?'öôìæ®?âS3?Ñ?ÉMûá|?ÒzI€/Bì?°7ÿîß²ˆ?³åÏbb‰?¢""&­Î6?äF!S{–é?±06ߨ+4?áâIêH¢?¶Ó9Y<j?~@R±Já¶?w¸]õÁE?ÛÂî![Dt?¶³;-tú MIXED4FGL J1716.1+2309?ÞÊ8/=Җ@>§T~–À:}ÜygËÀ<~¾b¦¾@ 4‹Âktî?ü‹vUDz²?Ä1}{€Õ?ÂFÒâ»vŽ@F}ÄY?ú<–÷RÝH¿ïiaB?ïÿîbHÊt¿àVà¡ë͙¿Ég]äâî¿é
Ä^ê<¿Çâðµ	UNASNone?ïX 8!ã?–xòp§0?hèⱀ`!?dµzÊCT?'Îܨ>
?•žÐh¢P®?ï#K÷¥='?–^=`ô²?ƒ´¸ãÂÐ?ˆv2¨?'¼s´
Ö[?ˆfG_Ç?ïÞäî ?Ž"/m0?y¥×ÓV¢Ñ?`=•ªQC?–ú­'EY?‰e4šãÝ?íQuàÏ/ ?‰2Û Võv?£"èfïì?s#´ ;5?§c¹ˆ®W?M­_Wª?î½V†¹0ý?žæÑ·–zm?‡ÃÊ8«"¯?ƒ$÷g÷QX?œsJ
ÌGþ?œìDÔsÉÌ?í¢œ²Cß?¯Ëƒqp!ÿ?™œ˜áê"?£QK¤¨A?©èl:Ë?¢4˜8öŠ™?îR³"
?—²¤,š"?‡©½Í,My?†­û_ä?¤ì•Y·å?'Šv©é?ênð"A? ¼ZWȏ?²ã¨ØèC?—ÛéëّÞ?¹¬7ŸH¢?–5ÜÌBeAGN4FGL J1716.1-4342c?Ù<£›oÜÀ	U°5½Q/À9§>ïÿ×¼À:îfWLíï@~Êö†@¿–áXu?ÒéWG²J?ٗ֠áž@
/Â=&Ñü@-ø¦š^?ï
užèó¿æ"_@Ø7¿ä˜=Î펿ëÉZQ…-Ò¿äس|
¿ïÿäÅøUNASNone)?Ѧk×i‰?¡Ïè•f?¬îËL-·?¦D˜S|"?å^˜áÉð?Ãhÿ–ý?ݒV^²?ÅÔpOsZÁ?¡#c"Fjë? ;@ž°Î¢?à$ƒö"(?Ä¡Ðêé˜`?Ú	 âŠ7?³'oA•òQ?º*å±Ëº?£}|ÛÝ[Ç?ßl%Ïê°Û?³aó~×`?Ð/_Óiù?¤h§¾ˆW?®•¢ŒXÿ¦?‹
[A?åþõ퓧ù?¥DÀV[
?ÄxˆQó"?µ‡J¡?§A#¢ Å«? À8uÚ{ ?é‡O¤í`?¸{Vhþ'c?Æ3ÓÔ	5?¿þlÓ¤«?­N<[Íq"?¯'9&Pòm?èž'rW,Ú?ÀÓÑ"òÉ6?Ë֔+›=?¬*
Ài?¼p
¿v¢õ?¦P"øø?å|Y*GÒ?±ZGØEv¹?´Aã/áD?•1·—Ǹ?°}Ø*]}ˆ?—g0]7`?ëh"›zg?ŸV›rUÀ£OTHER4FGL J1716.9-4152?íAIò<sÀÖÆÞvB|À9½laR*oÀ;"÷í@'qÓW@7"¹hkú?ÍWÙu&É?ʧ"Är¶+@j <¶i´?û†2(œ+?ï5¹pޏ?ïg,_›–¿ØÝZ»g¿äE‹àsr¾¿èªÜb§¿ïþîB=g?UNASNone?ÒdÞÏ·@|?Å®ÑÄÙ8k?•°‹cûñá?Ž½8×£D²?æ =-»ƒ?ŒQhtÕâ?ÖøVÚ?Ãöe.z^7?¥Vgã
ž6? 3bH«ˆ?ã›vÍ*¯?Ӏû½ûú?Ü«kÔŠ‡?³¢Õ7Âs‰?­¿$?™ÖÓ[¾4?ߜ³IÃîW?³$}Œ€~?Ôäk§Ù?¨æÖFõ½?¼Ô8¦å‡"?š^ÓWÒæ?áóp5OË£?«VÕòåo?Ã/Ñ~ã4î?¼cÖÇ«€?£Æüçb;?›mA³ñÇ?é÷›Ññé?½])b
Gh?Âiü;-O?¸ÕGÃÙ¡+?«LÆ>S§ç?ªW¥M>è—?é°´]Bž?»¤D5—š?Ëû>Ã<Þ¶?®$páªÚ?³°ÌÈè^?ž¼|6v"‹?拶¼?°¢¾µ¡¦È?ĺ'+6°?¦ŠŽéÜ4ñ?À䮯š&?¥Ök¬Ù½?æÎ"‰†•Ë?°2À[J4ŸOTHER4FGL J1717.0-3218¿×Z‰»w‡B@
WýO0ÀÀ9älòq¢À;6q'Šˆ…@ íãLì@¡ÞËÒÒ?Ã*[sCD¿C10ǾZ?¡ñ,}ŒrÀ@Õ®zÒ.6¿ã'㍲b?ïœ)@ìt¿å,"½ð¿èó`_fAþ¿èkÆ¢'9ú?¸ˆ_	¥Æ#UNASNone?æ§C¯ht?Á`ûöä?mN´v/­?f²
a*€?ÒvÜlõC0?Ã}þaßû?ç¹s{o.ƒ?Ė(‹dw¤?'=
ÛÑч?‡¤@©¢Ø?Ïöaeö~ø?Ä4ŒÆïµ?æ9Ÿ‰ü ?±U)âƒk¦?—d[õO¡?‹¶>×0qñ?Ò­²f?°ÒD-ßê¿?é¡R ‹Ñ/?Ÿ3©š"v?'ºL·|¥5?fmf‡A?ÈO²2uQ?žm»‡d"¨?ßJËÉJ>ñ?Ǻp¿/Ö1?Šï:ŠëUú?†4±›?¢\?ßݺb^f_?DZ¡ÚìÜ?ád7£–ƒÌ?ÈÉCš"?Ž‹Ýáv?š]‰o–@?ÜF·Õöœ?Ç{+ÔÀü?Ù\,õ	4?´G`Í~›?¨ú˜©"?˜Æ×´?3Þ?áÂA‹—g?´‹Ä¼)‰?âYž÷e?¯Îoßò?"L<-R«?'6 Ç¬™?ÚÙþ…ùÌ?¯PçøBžMIXED4FGL J1717.5-5804?ígšlíÀ'hRÀ:kàèãƒÈÀ<~Êx_@G2?˜F]?üX#ã4_?ÊÚ*BôœJ?èð¾C
Â@5I¢
c@¥®¥ÅL?ìMIÊNmK¿â¡Ý_ìû¿•ˆÞWÜ¿à8IÝï‰æ¿ïÆd""T‹¿ïý	«zl®UNASNone3FGL J1717.6-5802?¿8ê(
¡d?¿a¥®È!d?éAŸ>
´?Åo gÐ/?¶ºèeoö?´c}Ѷ?¶Ô½Â,†?·ƒ½ZÜ?â"ö<õ?Æ*‰š·À?Õ$ë㤐Õ?ÅSǎ…¥'?Ê/®jd¡?¯í'[Úþ?äàºü{ø/?´D-ëñaI?ÂMe£óº¢?§pÓrpo[?×·‰‡[\%?ªV´Þí¬X?ܺ돫?°*´^–ä3?Çdìã? ü‹?ßu?¶¸YG¥ù?²‡(gæ×?êÀ8â-?¾ÛJ¾ëÔ?¸¹âá_v ?´¥Âé;pÙ?ªȜ¤V…?°°ÿÔX~¿?ä†ÏNԛÆ?Êó€³?Ó²HO'§Ã?ÉËñ	üÞ?¿oJœð¼?¨•C¨ß"^?ç©ÅÎÖ½<?³Jq°tç?Á¡C|V'´?ª£nlŠ»Ý?Å4©ëKh?§R_÷¡¬?â},iH ´?·9PYüÏ?ÐkR6·)Ö?°j¸£­ÁPSR4FGL J1717.5-4022¿ÁnÈ=Nž¿÷SŒdý±À:–Í[h£À<Br©jÈ@ B–áÙNe?ÿƒ\=¹?Õ2køvžÃ?ïùƒ^ıu@á¹Þ³?ý:˜‡ É¿ärâ?û˜'¿ïÿä†ýµ£?ïþú·Šñ¿Ø‹*k
•¿ì°¡óÛ/¿ïé˜_‡ÏîUNASNone?©ÀÁ³ùs?¯†gæ'Ò?·'Ø¢´n‰?· (8ø&ê?ëqÄß©¯x?ÀdÞ¼½'?¹R¾¨Úšº?»íT›|?Ë(ÃôóË?ÄQŒt˜?æw-š(F?óBͅŠ?Ø1z¿lo?²©NÒÒɇ?Ò0/Œyd_?±IX#?՞U´,?²qàhÇ$þ?Ï£Ê#hÿ?¬ù~]?×_§~ùI?º"YÏæBü?ØÎsoR7?¶Br0$A?šîùh#de?¡föÚíjà?²V¨jÆ1"?³ÒÌ,á+÷?ìݳ'<ãi?¸ð™]±!{?¤U§A1?­¸FŒd#?Ék*ƒ¿Æ2?ƛ¦ç,kæ?è_Úæ7y`?ÅÌ2¹Ä:?Ñ=ziA|?±ÚgÃbj?ÔSçñ1l?µJ^Ί-?Úo"Ý¥?µü‡>g»?¶ó*‹m&·?¤Â˜dÆ?Úú-.G¢<?Å$® 'Û_?ßI.o —?Ã]
ë-¾ˆMIXED4FGL J1717.6-4404?ÏÙk@ÀºpÀ¿¸fä;À9"šv8kÀ:Ûµ#bۗ@f_>ÿÅ@8Z\lèa?ÒI䥆?ÕޏÂÖ(ì@Dy¬"H@n"³*å?ïüPþ .‰¿íQ9®ww0¿ÞJªž#Áü¿è¬Fàˆ¿ë•¢ß='³¿ïúÂÇ;=UNASNone3FGL J1717.6-4404?ÃÌ·'|‹[?¼ÂΟ={?À»ïãZá?Î-!eN?æÜ##hq?̝&™YF?ÝÿüÑ«+?ÅOäW5¤…?3-{y£#?šûŒæžS>?àh+"àq?Ä~IËL?ÙóL.h†?²'S¾PÚ¤?»¿éöz?¤…`DÁه?ß¹Sôõ?²Ã4N!‡J?Ñ¡ŸÑ?¢Ãã³Ý×P?©JáÁÅr?…帹Áî}?åà} ?£Çø‹CIê?µ4Ø9Õs@?°X@;	?®Æ2l0?¾_.èåv?ëmÐå‹5?ÀÛù¡¨B?É…•«£\?ÀI¢Q_T`?¦À˜äwjC?¨±l£[(4?èRUvÛÔ?ÀÜz¿;Ù?Íݏ¦gò?®H3=¢«o?»ByR…?£:7ÃE"?åóÔoû³?±''-"º?¶kqD|5ú?•š56Gٖ?¬n[°ÞbT?"`C¾o?ëk¬9WÌ?/±HŒá¥OTHER4FGL J1717.8+1955¿å3]oÐP@=1	¾ºÀ:Ë:CȬ­À<bw‰¤Y@Ú Gs1@éºÿDï?¼Ö_Æ?"žgšÕ*?À†D}2…¹@¯Sj5S?CtÉÖ¿°Å'<3¿êþ'âÆ3V¿èdµVŽ'¿«d]D 7пè™ÇâWMšUNASNone?›š·?‡`°5jÛ?c]µR0É&?Yn,ýeÑ(?ŠÁïVÃ
å?†÷ëH3?ï ^@
rk?ƒEKô«$:?`µW­ÁdÔ?g™Æß#ÆÂ?ƒ»Â0?~n `ü?îéeü?§6{—D
?{5qÝ+)?z1ÒqS?›÷&‰?ˆôLjWam?i"L?fNºí»?V´1
¤?EÓ%ɖs?"åÖW;Û`?d'[SÏ?îáñOãî?˜XcÀyz?yxŸD
?urpûŠ¹N?š£¯È;?•ÜøU?ï7Ñ-Ä0?"º•eøðQ?g¡€Ì3l?uUØçVI?–·Ò-£–?'"¶h®Ör?íásîº?˜fô݋V£?ˆ¸eŠéë{?ƒn]Ÿþ¥?«µ¼Ãrä'?•YSÍ?_þ?/IŒ?†ØY3R0Ý?tºŠWÕª?kmŸÿÝðß?¡ð[¼!*ˆ?"Ë)ü¬"-AGN4FGL J1717.8+3925?ßfïç¶@A†
¢À;Uî:ތÀ<ɓnÝ-m@ ïñ2@º­,**?ӟ¡[¢?Û>.cëŒÖ@û$ p¸Ð@¶ÁȌ̿ïýíÁ?￧¬_o¿Äó¡ã?*¿åB˜Ì@)¿çï…^y2¿ï¾­àMˆUNASNone?ï"Kٔ¨»?ƒŠrÝ\¯á?b";$wk?[ñtXÉó?†¤zÚLù>?'s"/{"u?ïhv1|?Šý‡MéLG?tõ çOß®?wÇ¡á8?‹g‹½S3?'7~ÀÔ?îÆQ²ò}ƒ?'û¾=BÁ?†Õå^ÅÜc?ƒ$Z»×îÔ?›ÊÖù,™j?Œ˜C40~æ?îq¾Ü}?€K54I››?—N¬òxH?tjf¹_?šÐwd+?x¬YK?ï<håWï;?‹ÝÚ¼#²7?t/ó‰ŒG­?pþô˜ý3?"fæv¾Ž¡?‰…a-‹a?îOâIwà?£±•õM?r'=­?'æÀÓj+à?£¥:ñõN—?›……ÝÇh?íÀK£Ü,€?œ$c=O?"ç£Í+Ì?tA }F?©‡sÞ;b–?•ÎçIÉÏL?ìjM£÷Ám?˜v-G¥ŸÑ?¥é¯«…¨—?ŽrY"'?±¸»
íË?"]^NÁñAGN4FGL J1718.6-5821?êöÿ¨rÀ'ø@À:
ùûAÀ;ǁ]b±¦@Õ0‹yp@}G8£µ|?ÁÙ¿¤p7K?´hÊCÛw
?ðŸ-݈ܳ@•»ô7tá?ïÆTdÜ#¿ãªÛuÜûï¿æî!7¿äNMÃiÍ¿îÐüqÖ1¿ïîDنUNASNone?ìtÕQM
?³)tÞJ?"B
y¹Í?woú/
æ?¹×m5s»u?²¬aáۚ?ën¦Ñ»t?ÀµýR{£?…–HË-·à?‰ê~
2c?ˆà×Ï<ò?¾ûm§«Þž?ëcMÍñÅ?©`«›·œˆ?ž~î…t¡?'é%«²·'?½EÕ°?¦BÄëܦ?ì©·îæŸ~?J'æÆè?š
^|ñ+?x#ÂË>Ê?´/¨ë'UÁ?‹%°BòP¼?ꛥþµZÉ?¼×Iõ¹Í?–/–i»ò?Œ0´èOk??ÂËu8*,¾?»@4ߖå?ædC^N"ã?ÊøK¯ðŒß?–Téû׈Z?¡íL%âG?ÑÒ*£ÜWs?ÊGùÞd?çŸçÞ9ö`?´f½Õ1L?«÷¨y£ˆo?›+,_S?ʂvgeiç?²ÀqUÊæ,?èœt.??£¾‡e"£H?°k^rd?"
?p™ D?ÇnTÆD·?¡aÈ2›AGN4FGL J1719.0-4038¿²níJ
¿ýeÙ($â8À:|Í°ø[À;JuòËd@ µY€.@aøDIÜ?ÇÚDºõŠ?¦C®Öl³²?å>ÖÕdK?üAòMå¼?ï­o¤Ó‰¿çN>f˜¿å<â¿'r¶¿å]'«ŽŽ¤¿á£Ž_©³Ã¿ß1ßá|‡:UNASNone?Ù²ô+³?¾UËtÄ3\?` u%Nù¢?OX£¢$?ãeuXOU?¾`‡Ge!ö?Ùêê<§Ù¬?Ç¥ÑÝÅ?‹÷e4‰µÑ?'êž8{!?⚭LÌ-ã?ÇMÄÍ®‰?á>C'¿@%?´Ytƒ"%•?'åb[Da?½õ	Õs?Üe"ԖDÐ?´IAwЎQ?ݯU—zõ.?¦¤!nûæ_?'äÆ^`Âê?sÏ4‰10?à™/†y?¦ÌŒ¡h¹á?È÷?³±êJñqÆ?hUìÝz?[[E#ŠCœ?éç¤ ]"?³Ðbç''U?ȕoBn?ÀÊp«âÙ?ˆ Öþî¡Î?"UÝ1gå?éz À>ôÝ?ÀÀ'ÃŽÎ?ЪŠÛÄ??²e"
aÎi?˜WK¾_ñ?'ÿ³éÎӟ?æèLjó¸?²˜Þ'E®Ð?È)÷æ¼?¤8@?˜Nd°çe–?†˜ÓH8?é3Eœí6$?¥¤Êÿ\ýMIXED4FGL J1719.0-4221?ï
äAôyÀ v}4ßÀ9Á•XÂ8õÀ;A	pÂ
@>nfë@C{Ó?Î!4x®?܉+bYfy@LeáÜ(Š?ök¥¥–}?ïmq½²}–¿x:ì1ŽdÕ¿åYxâií¿è— Ÿ²¸¿ëɉDH"¿ïó<7¾³/UNASNone?Æ®sn?V`?¹_Š'X?Áàz $?´»ÅQÂ?æ+è!g?À{ƒ{l?ÉÒӃí'F?¯TŽD?Å!'9³K?»^>öF)?äBæÐÀ2œ?Áú™¹¤ý?Ñ]¶æÛö?­×™Då+K?¾¶þ2º+N?£-¿rD‹¸?ãzDÇ&¼û?°»Ø×ɵS?¹ uƒtE ?$}ÄÄ2?ڍ)d—?§uW2U;?ß*áuPd?¦¤2ú©)?°ª¡ªT)?¤ÊmLä©?À<®'Åþ¹?µÄ"À¨Š?éۀ)Ž¢M?¹$RÞöÐ>?¯~ó´™Úo?¯t»"\I£?ËT?¥åàÎ?ÃóDæc÷¡?ç3Û®Ö?Á+wÌÌ?Àϕ5ÿÝ?¢zcëÏ×?º÷ðÚÉ?¥`ÔXcL?èm9ôdã§?®YœÊ¬?™ z—}?z°ZXïõ?Ýê9ÐíT?°ÕZ' ¨?à=ßB´õ/?°{¬»ã°OTHER4FGL J1719.1-5348¿ïvi?x²À"¤w¯dÀ:hRGËp¬À<¿¨!Ù@…"|NZ+@–žh5s?¬Gq-À?@‡1Ó?Ñ´âË;Ó@×nŽ¨ú¶¿îJj½
<)?ïò§½HËK¿Ý·DdÞÑÝ¿æ'Ê !Èþ¿Û#¾…â-¿à9"¿ºëyUNASNone?é×Ãd)†r?¹ÊLÌ®¼8?ƒÕ "Xkã?yËëqÄ»¡?Çc˜fúÇ?¹@ûк?í¡S^?µ1gÖEû?VípÞõÑK?aSIVŸÄ¸?²™ª¿êbË?µHfµ?íß®j¥Õ?Ÿîûƒ–
x?ƒšç
‡`¼?}é$žQY?µ-¥«zá€?žG	«"»'?îE²ý?'%µÙWªû?t€7'T+ò?ZÀ\éEl†?©è.šJ®?aKcôx»?ä¨SºÖïÕ?À‡<n_?œù¬²Xµ×?'ü.ª±p°?Ôß½¿,"ø?À:À…ª?é­Ô?™X?Çdîï-í?eã?š¿[?sÙpÜM~§?Èñ"WoË?ÇVޓɠó?èº\ r"_?­Àš\´¢9?"°ø°ÖL'?…·±ÛÐbé?Ê nh$ý?¬¢Ñwg¦¿?ë ¢*"$?š&'±õ°ò?‡ú3dÜÝ?vu¼Eo8±?¿û¨AýüE?™ŒvªÞ
ÝAGN4FGL J1719.3-3424?ëü¼‡7õÃ?û!Â]BÀ:d%B{¦À<¦Á Hà@ƒžçŒ@Á@ľ
'*?ՈŽÄÔZá?ïú›ýwª@'
=p£×@Âè/SՕ¿ä‡Úà
í¿Ó§üÞ¸\¨?äz؍Út¿äém
A"¿ïüª£´P?ï@ôQvYUNASNone?¿tCZé?¸H_+F›?̹Báüߺ?Á¤ƒÏÐ/?äã&Ü@eÔ?ÅOOëÈ?Á>!ßßà?Â+ïíûb?Ò_8Kî7x?ǙB¨©?âŒTQ{í?Éø€Xà?ØâSNS ?³›ŒÆž÷?ÑRRw
k?°OFz'â(?ÕËZ;µ¸´?±·NÅNÂõ?ÙÂ|Üõcð?´^í8a¢0?ÖÆÛY‹N?·Œèí½þÁ?ÎíO•$Ñ?±¼±"?­+õœÕD?¨X2Mˆ?ËǶ¼¨µ?Á±_!èKó?ç;S"fÝ/?ÃÁ&Anp‡?°ÔllŒ\?¸1Y L•?×[í¼ I?ÏGZá¼·Æ?â7ó{¯›0?δ
ýÁ§?ËgċW.?­Ú0=®ý?ס'ÇàvD?·"­?•w?ÚªæÕÙÞ%?¶¤Y8#µ?À›oÐ¥ýß?«õåvœ'?àj™i$ÿ?ÁÁ†Rj,?ÖÝEr·?¿™ô0"òMIXED4FGL J1719.4-2916?›nÿ†Tç@n"$咖À:Q'l~®\À;UÎ{"¶
@!uÇ,yÜ@E¦'¶(F?Öââ7î?Þ¡x ¥§o@ ˆC0y@YKË°m?ïR…sq礿Ý]+4¾y¿ç˜Æ‰ˆ*¿æ¡^X¿îÚÑb2Ð¿ïþ*ÝúºUNASNone?ÞÃ?Ã6æ?ÄÇñ%œœ®?«!{$s? §ƒºz³Ò?Ýؑ†Ð"-?ÄØ®¾€?݈áNÊW?Ãjd œä?´ðÖ?Dìø?®»ªóUš?Ý:éWijÊ?Áªt䔥Ð?áç,Î%xœ?´ÆXý7ÇÄ?µfϱ/l½? .i µ?-?Ö×òwM¶º?´5‹obÎ?×÷ñUd­Ì?¥0Èì4Êw?»·Îèі?—ØIðžj?à
xIÎç?¦ºÍ'úì?ÍVMí>?»™Ð‡R«Z?»†©Ž'n?°áà*›¶µ?å9£ẑƒ?ÀÌßæžÉÉ?ǯ‰Í ?½ÛLJ¯?ÅF»®ÊáÄ?ÀÑu¨ùˆí?äŒ2"G?ÂþCg]Ý+?Ó«ÿ+ˆˆ¿?³ºÖ¡ªÃ?Àñ¨Ý9ñ?¨€EÖÇú?áí–BÄm$?¶Ï‰UÆß?¿&ÄzmÚN?œþHÎXœ?ÂPà±õÊ·?¨T\+W¥6?ç†ïD4Ò	?ªïwûê±MIXED4FGL J1720.1-4358?â
ܞ?àZÀ<Á^ڀêÀ9†¿:¬¤À;$G4q÷"@á›þMÎ?@…ÜMsP?Æ[yMsÑ?ºþv½÷qç?øýÎè/ÿ¢@9öw– ?ë0¿e†?ïx5›Ã?…¿éJº¾­OY¿äËZ;µ¸´¿àqÁŸ:¿ï¾ÿ—$tUNASNone?ß×-ÖIo­?Ç¢!ˆ:÷x?ÉMp´?™ÛóiX²?ß Sފ "?ǝ‡º;P?ãó?ÂXªC¾y?ŽyAE«Áö?}áPi.?Øà/ß°n?Á—›ºÓr?âF‰ïC?´BÏ&|6?¡ þ~$çú?'OґŒù±?ÙNÎ ?³z¹jÖsÑ?゠ÍP¼l?¦EÊI×é?©é#²?‹<¢ä=Ú?Õ½šõR?¥'ˆnÉÃJ?Ж"ß±‰ƒ?¿¡"SU×<?Ž|"ôÁ¿?f;Çw?ç:þÜnx?À8‡"ù»?Ô 4ÎhÙ2?ÃMNtN¨Ò?›¿ Ì‡—?£'íDadç?å쓳óÚ?ÃJäsæ	?Ó²2Ë6þ?²ÌÚÇP%?¨ù$ą€ˆ?"‡ñlšM?äéšRx?³d…z»£~?ÖÍ&_¡au?®}i85£?µ¹{EÍgó?žÓýF%ùñ?áâ=g>¨‡?¯U«H¼´MIXED4FGL J1720.6+0708¿é‰§wíf@7kDå^³À9×Ùµ›äÀ<àŽJ°þ@´fêD×Ë@Yܚ )×?Á#Q(f¦}?Ù é¤@ŸË':)Ç?þ¶§NŽ?ïý$ƒmj¿Ñô;[uǂ¿áäÊE¿ç|卍ó¿ìÞÛÃ	Õl¿ïä1‹@UNASNone3FGL J1720.7+0711?Ãe1Ÿ¬¥‡?·ç'éik?ãf
ê¾:?Ê0†Ҙ?Ï–µ[
?ÂÚû=+7?Äg ¾šº?½ÜÃOu‰?çéäï¯Æ?ÁE-»q?·â—	R[?°W¾#øž?Ç
Aö´@©?«¨V@?âwª|Ñô?³$2`æ¤Ù?Ï_a~9?®±žxD˜?×áݳ­u?¢½Îö8~?؊è;¿?¦uVüãI?Ðe5'ÁÍ? é:¡Ô‹?³°˜¨q½v?©w–\Êǔ?æ$ðO˜D?Ç(jò'?͓óZˆÀ6?Âƕâ;/<?²Âe¶Ã??²Ò–%î(?ê·¼ck¬?½M¶ Ò¢?··2k>?±Åk9Ê?¸"qw
>?£B¥:8jh?åGiK¦¥#?µAñb]Œ?Π"&þr?±äƒ"A¢?Ä/'ÍWê«?œ+vϊÚ?ÞäS>ôåù?±H¼§¨.?×ëZ_$±?®"ŽcPSR4FGL J1721.3-5257¿Ýb¾"Xo¶À"AiÂ;ySÀ:%ÛÞ¸‡›À<$"û¥'l@
5]/@ô·Í?Åï"77y¿?ãªØ¡e@ëÒú
w¸@Ù¡û½Ñ¿Ï2þ'W¿Ý×&¢¬ì¿ÜëÀ š¿é_îbHÊt¿ïôù è­Ô¿ï%m
ÊUNASNone3FGL J1721.4-5253?È\e]Ê-?·'(r¹%¾?Û9Iw­?üM‡ó)?ؘÍýqÓ?ÁQÅi¹?Áöû␅?½.ÂÊ £?ڄ­Tȕl?ÄS˜ÃÛ·v?ÜÔº4¢R?ÅZÃФȢ?Ð뺈Òw?°iå6
Ä?Þðo±59?²ü½yâ]ò?Ð#ÕÅøOæ?­Ì	"q'?ØÕU/dû
?£â¥³«?֙Xž0?¥{™ûÕ~?БR2|Ôè? °Êµ0Óü?¯š
Z[r?¡¥R'ý{Ê?Þ£
Á¤ûx?ÅãŒ[1mÐ?Ýi³óbå?ÅuÏS?±àB0JL_?¶"kä‰êÀ?Þç÷‰þŠÏ?Ë$‹£j[q?ܟ÷éÓe:?ʺé'\ˆŽ?ÂömQ‰'?¥Ç0D….í?âmh°÷§?µþ˜¢:â[?Ò3h7Kò?³+GcÑ<œ?Ã[ïÆ]->?ŸRÀÙ<?ß1PÙÑ?±8@Ѩêõ?× ·Cc[?­K"wnW"MIXED4FGL J1721.4+2529¿âó]òÆÓÜ@>?§e47?À:sÿÜĒÀ<DTž½ÅÉ@Œ¶¦Å§@æù[¡†?¤#
q¿¯—%ÿv Ï?å&-'2ÂË@ú 
÷Õº¿ÓÀŽ%D.¿ê–-žž¼¿éÿ7T*$¿çñ"'›¿ãæþÜêQB¿ïæH¿™UNASNone?ïÀ[Tºlx?­ꥺ_?boÕw)¥ë?"¼4ZAî?všjü'"ñ?¦M+uÝN?ïÂ"^ë?ƒ'i.ú·¿?W™_ÊÜUÙ?lðvâsÌ?y
æ•´ã?z¯5dŸ< ?ïA`ŽÏ«?"Û{E®{w?kNoÄôê?i¯º`šm?"s&5N?ƒfË°QõÌ?ïÊ/z°º?[^€,Õ[?Wñ?øÛ?BÄ25º"?tëòçD›†?W#¢¸g8?ï¯À†Ó?™a»›qìõ?iی|2?wZÒ@ú{?{š¬p?"¯åǀÃÆ?ïWC@Ðr?•!Âfz/?gd&ɂp?z1ÞLŽ'l?'+°Ï?Îé—Î?î^‹‹¹Ý?"ß "Ê'?|ÿAo>‰?unçYäúu?¦w_ß÷Q?'üm8—Û?ïJrŠÖï?7«{Ž?v`¼pC?iŽ] Mš–?'¹~U4T?y'IÙóAGN4FGL J1721.4+1131¿×ÉUSÄx@@9$ƒÛÂ3À:Eóå?ŠZÀ;íåf ÆI@dˆSöø@('»0Ã?Ä\|,Ì<?µÛ.dlf?ñúÑ!Æ#e@Ley+ü¿ïä:Âs­w?ï´êB~¸¿â7¨ã¹x\¿é¡nD9Q¿Ü4Â_5š—¿ãƒö.Åæ)UNASNone?ïA.-1]è?Š{¿Âaߥ?f)nf?Y³Ìp°?•u!39:?‰GÔUd.?ï¨tY?'pÓ3}â?`+ùŸêõ?fë=&¯GÓ?âí/λÄ?{̌1½l|?íÞ±fÈi™?š³Ÿ
Ó¦{?‰¸r; ƒÝ?ƒ)¹Ð ?«¦Ím,r?—IëE-¾?î;Y"í&?òäûÎG?'c°½]O?hSϬñP=?§±£ËÐ?ÝÙR¬Ì-?îwƒôä?™2--Å?{åKúÏqq?q,lŸ§?¥6,«½?˜˜ˆ7÷‡?ïÈqߎ?—Y®
?sÝnúsÌ?|M'ï>?š¢5NµS?"ñ|°>r?êÐÀê7ä?«Süg«F?ž]*+lQ?'ðÎ+>?ÀñW,õ¤?¨	çõȳ?ëe­'?ñï?›´¿ü	g?–åî+Î,L?…KË_|w?¿aÃ
ù?™mÞ vçðAGN4FGL J1721.7-3917¿ïÛ}ä ?T¿÷ÝÚ;JXêÀ9Pè0-À:ÝîgQGñ@•8"Djé@7褙§Ü?ãRÿ" ?Ð÷Šûñþ`@À ìߒ?ûË …¸Ò?çi·ßTä´¿Úzµ]šdñ¿å^ê–p¿àuT«Rÿ¿ð?ïþ¥¢fqÏUNASNone3FGL J1721.8-3919?…€ÝàñG?ºæcæ"Y?ÑDÏ4Rf?Æ	eTéU?â¼8.^{û?ȗKÖÃÇ?ÓˆÓÆ?Æd¶êH™Þ?±—P)%LÈ?¬]Kõ÷¾h?äA†61Ó?Å Q<?Ó1È ©i'?°Ûá\þ=?ÆÉsQ?«Ï.ŽÏ4]?à´¾Ûiêø?²Íi=*?Â-¬ØÝõ?¢`¤23_Ò?¹Åûú_,?šHÛpfŠó?èCµ3J|?¨LÁvB׊?·çèlqŠŠ?°§¾ÅÍæ?Ðn%AØèd?Å`Š=?äËðQiݝ?Ç^7¬0?³#´­J?²Ùyu»-?´ì
ô†£?´¢ÕWøÉÝ?êò[üø[?º2‡´WD?ÇVLgâ'\?©êNmðJ5?Èö:':Šô?¯2
9ìŽH?ãìÞDïHM?²ˆŽåx¤³?¢
7&ââ?‹/³Y?Àh|øñeU?¨¤ÂÃc¶l?êÅ`£¯?«fXuH<ÁOTHER4FGL J1722.1-4007¿çÌMyÿ©À*¼¤¡5À9q¼´i)À:þX"»@=ó~'W0@µiF·G?Êl‡"?Ŝ¢x†0@Bõ:ªú@ͳ\cX??âøC]¢Èl¿ÜQ0^ƒ¿ä¸Çâ'@¸¿âs,þåÑ¿ïOÙ\'H?ÔVˀœUNASNone
?Ô.çÎI¾T?Å)£èR?šSàí?'×$Š;?åï"çœ÷?ÅmôTƒÃ?à²Vî"
?ÅO
¿¡–?•âSéZN?"HӒë}Þ?Ýfy|ÿÁ'?ĈaãÊÀ-?Ý诲ÆÍk?´«Ê€Ž¨?¬â]nûHQ?˜Þ¤5Šî‰?Þ{ŸRì?´ŒÂ.ƒä
?ݛ=£y—F?©"föKy»?£ý1Jy®?uÇH¦§g?ßå3LE?©UE€Zì?ÄD¢~<w?µ;­¡©Ø?¡MóiI?˜:å⦖?éÝâ?Î?·>{V[®?ÉõÛP•'?¾þ¢-£›?œÍÓ³îÎ?¢þ®N.?èœ"æ7"?¿SáS—¼?Í/êm5|R?®"•p*?²ˆìÓ´dÏ?›É0) \W?æbçÊeO¡?°a2"é™I?ÈB•«U?¤™F¤´gÂ?­u'sø"½?'Cbˆéў?èm॔?¦"
§}ü¾MIXED4FGL J1722.1-3205¿í'+årFU@Mt­P0À8Ù¤K¤CAÀ:³*dW˜m@ñ+:ÁG@ø¼²£V?Õ²½?É[¼>_@a~4¹E1?û/-4k—~¿ïr> wæ?ïýéÚúŒù¿èÄ¢'ßܿ䅠ž²´¿è)ó¹  ¿ïÿ´ìw8UNASNone?Ñï'ÉÒ­ž?ÁQôr
çî?´¯Úù‹?°åó³Û(?ä"tÅ`/?ÃçåíZ6?É%µLû—?¾Â9éä=_?ΎD±ŠÒ?Â%]Qê®_?␜;?ÁµÚv2?Ò,–y²&6?²ÃnÃØ$?ÄF¶:íšU?ªëû"Mà'?áØ3âð?´r(ó[…K?Ç@nã–'? þñ}ªQ'?ÂsQñºB?šˆòé'á?å"Ê«èÚ?¦ªm¦qz^?ÊøųÝ?¼Í ¼…yI?½:Úq{x?´™\+"Æ`?åšsDur?Ã5ìÿ?´[S…ü¼?²+7½æ½Õ?Ô¢®‰Hq<?ÈHGÕµ1X?ã#>X!Ì{?ÇÎF"@8?É*†ç:aP?«ž«ë÷t?ÄÝFLj'Ä?¬¯Dï¦Ê?ä~³ 3š?³6ê$¦?²"e¸"?" ¡hÎ~0?ÇÌðd'·ä?¨yÁ5_ ^?çÊsYûT?¬ƒ~"}CFOTHER4FGL J1722.6-3135¿ïå¦åd@¹^ƒCÿÀ:m^º z^À;üVÈc±€@XýËrYº@Ú³R¨D?փže[N…?îù¶9ãP@Z5Ö{¢?ÿ‹Þuk¼ç?ًÛk¡¿è×n~ÓE¿Æ~h»«<Y¿Ü	ÆTㇿïÿý{ÁA~?h$¬ˆUNASNone?º÷âÚz?¶½¤†â¦·?Ò#9,~?Èfö?ãg:Žr?Ëh7vä¸Ò?ÎCöò1­™?Éh´pÖV?ÑTb+Ýî!?ÇÝJ‹à?߉¢[	;?ÇÜ7ªL€r?×þ9•¼¯?³¢¨gæå?Ó.Ã%ÈÖ7?³M
ݚ?ÔÓDzz½?±Kßüè9?ÏÃ56(?¬½–­ˆ?Øý|W"f?µœªCî"Ý?× éQ$¾?³Šc6ÂE?¯´©UÔ?¨ä$×J¶$?ÓMǪ_JÏ?ȘÞ9?ähŸØ;Û?É¿g«B?´X0P|ZŸ?ºÎ$÷ÂU?Ø)/v¹Ð?Ï1ðéÀ+?á`b;"¤?ÍNV5|õ°?ÌÔwõô¨"?¯Üß1«"?ÚÛ°•^¡?»õ*y{A?׈èTpMN?·ÀP6«'?ªîdjy ?—œ#vL™~?à@ßƂ9?Á?q¯ê?Ü"3"w¸ì?À©¾×üMIXED4FGL J1722.8-0418?í¹b"·Ç@1z¿¹¾ÓÀ9£ÎµÛÀÀ;ƒ¤Ùš;@Žy&²qW@òÜ`¾†¹?¿È`g¯ù?ȑXJz@é{f¨«…@d]!Ä ¿ïúþ8£N?ïþ|¿á
Æ,Ÿ›¿ç?!þØb­¿ä…ºŸM¸›¿ïÿõMõVYUNASNone3FGL J1722.7-0415?ìÐÐv"J¿?¯ýtfW™?¥D•KÐ:?¡	'‰Øg}?­ë´ßÑ?¤ê¡'Þá?êá«Ce/…?Á£p$?¹ëZI«"a?¼"´'Ä?®—8êwñ?¦±Òì
¿7?ç…tsšW?­ÝȂC"?³ƒXö^¼? ú¦tªi#?ÉÌ>-HsÈ?ª üc	R?ãv-
 ÇB?¢6ú{ÒKv?ÁÇháã+Ö?žÚŠ¢M'?Ð/ñtÌې?Ÿî
S'?è•,,â>Ø?¼KUÓµä?ÀàµÓÈ$Ù?µ¥]Úí?¹•2ðØ"?°¹ ¦\?ã"Î#…?΅úŠÓ·?Ñ8\ˆ`?Ì'Ib?¾€•¹²‹?´€'>Òá?â½J!Ðùò?²L­8У?À‹€ ³?§g`¿æèà?Ò|¦2ûÃ?¯â^¼öV?Õr¶	«"2?¨ã	ƒš%q?ϲíC úÈ?±EÒÛÐ7ö?Ú³ÓU–Ï)?®í/n²¯"MIXED4FGL J1723.1-2859?å4•3Œ@_\ÔmÀ9áºu²3ÄÀ;U';&F¼@¤š"i©½@ùB%?Ò*5}æ4Ó?ß<eáÜ)@ÅSü×V"@ña£Êu?Öû{8…ƒ?ïäÕ!…
ì¿ç²™0¬¿è:P(6ï¿ë»¹.׿ï®
4»ÉUNASNone?؁ÆŇð5?À'2ˆŸ?ÀïMÊ8H?³yðE/±Š?ß®'ó§?Á pÔº" ?Ô~ç`:Â
?Ä[b,×	Î?Ëï`ËqØà?ÁðÝg£?݉h:Qƒ?Â
ýþûÒ?Úzê<iM?²´<石?¿Çð¦éÞ?¥ëæ9ýŸ?ݓš'U|?³… :Ý÷m?ØíøäáI9?£‡#±q7â?Ð4:½žº?¥ÙSDªç»?ÖÝÌ]ü©?£Á u…,?¾Ì_zË	?±Ùԑ¾?È.݃˜?º¨êk)ç?åDË0Àg9?À¹2™¸×?¿ì~6u%?¹àƒkuR?ÕpëH¡?È>³Äèþ?áIú•2Ù?Ç#¾¼úØà?ȕÛôÝâõ?«<þC¦ï?ï½	,ÆÕ?­Â²§é…Ä?äî™À}UŽ?´ž)ç©Ð?ÃÊ)χ<J?Ÿ¿6#b·?Ö[2q¨u?³gHý''?ß¿¸¦"ìË?±g89h'¢MIXED4FGL J1723.5-0501e?ⱟk¯jU@0ös>»ýrÀ8¥½áw~½À;Gýœ@ sÍ$™g?ÿæI ]?­'—¾V迅'LmcR,?ÝÉn"æW@BØ(J¡å?Փë$%Ï¿ãÎý'¬¿ã©yámm¿Û1¢åGÂâ¿âCuÀÌcp¿ÆÑM$ ô,UNASNone3FGL J1725.0-0513?æàÝ9ü•?ă±]
U?…~&÷e§¥?zÈýxÓÞ´?ђT•Gi:?ÄG•¯˜ù%?ïí½C~?˜ÐÚô8é¯?{Ûãޑ¼E?ð'(¨ìü?•KO^·ñI?"¸3"€JÖ?â렇À?´p›˜ì-b?èÞ	çޗ?•
 'Ü;?ØJ1·?´œÂõ±¾?åK—€î/§?©$pW|>?˜5xæN[¶?t›€sµ³Æ?ÓåypH+W?¨qôFàÐj?æ
G|ô?À­9ßtÅ$?"U8ƒ¹W?"úû‡•ù?Ò¶R¯?ÀRŸêÁg?픛dcƓ?°$Î	›†Å?'@º—xÕ?ú¢5.	?­–C\wÚj?¨ÐÄÁû?à›Ú:î?µ"íµGŒ?—%6ìk-?'0Ò}2R/?ÝUøåFŸ?µn84'c—?ÛÂÿÇ©ô?²$fm?¦8¡?‡cµw"¸¿?ཞ¨ïo[?²\]"¢íRMIXED4FGL J1723.6-4126?¸†•[Àž'6§À9È.5p¿À;/51:4¯@'')Â@8M[Óem?Îàw	KÙ?¿ƒ"´µÕ?÷ÞêÁªYÛ?ã×vŒ#d^?íu–Ob=ã?čsñidH¿æIÅ$½ú¿æ—:yx'â¿æ™Umß¿ÌD87SÿUNASNone?è+ï~?Ái dgû?ß…ÇŒ¿i?žqã©${?Î5èڎE?Á^Vß?Ù£J–¥?Èt¤R¸½?§dNù¬6§?¨H³»îS?ḧ¨"?Æ]¬MPk?á'Mßÿ&?²Tq"ö?¢<AvXQ?'{$ÅytË?ڕÜȶN?±™Ár"ªÉ?ÇiŽúgÃ?œH8‰üq?ÂB@d–z?›:™T5ž?å"õ,è@q?¢%'…?݀VœÄÇE?Ƭr2ç!Ñ?ž_þL´?´[ՁÉG?àLÔ¿þ¥?Ɵöþ­"@?ÁpÙ˧¢‹?½ïd€¡ê»?±}ž"uày?´Ú_`ÒlŽ?étºb£?ÀSàF7ƒ?ÑKÄ2ÁÁ?°"\9Ÿ†?°feþä+v?Ÿ7¶pÔ?åM£Ýü[A?±8àÀ¹\ò?®.èûL?ßù´¾6?ÃX%»¦^Ï?¦ïàz@?éG´qü?§\œß°etMIXED4FGL J1724.5-3008¿°RÃâN†y@	aâs'?À:©¹¢MÀ;£­X"?
@Oe/Û@Á=¼#1?Ónä#Ösë?íÄÿxñƒe@zbœ­J?úbԘôF?ï^ mÿ¿Øꁺè¿áæ">iƒ¿ìªx^¶n¼¿ïÿÿ" 5•?á3Ê!Ì®oUNASNone	?¨sØÕC¾Ç?§#èü#»?´Y!½ì"{?³Â°ï¨M?ëíž:às?¹uI_¯?È$»ý'ÞR?È̺¥¥8?×`ŸÐÈãg?ËOkÝ¤Ã?܍0u­p?LJð¦éÞ?ÔsÏ	?°Ý3%H[?̺nŸß¤?®æëfO?Ý/¬›Tã?³¯òü€Q?¹»â˜Ï€?•ï‰o'Ðv?à*1¦Z(?°"Š(³ë?Ù<¤.%µÐ?®º£…yÓ¶?œCd{!+?¡šj¿Ÿ#?½ÁGÚyd?¹ò(7<éQ?ëZôéT›?½}û3œ?¯n)·%´?¹9™›öTÖ?Ü>DmŒË?ÎçkÝQ\ò?ßÓöÁV»½?Ì~βU'O?ƛ†{•ß?©²!§z?Ôa9—H?µ/¦LH?à(°BÄ?¶¸Î¼\?–íKú]?&썻I­?áVIJ«l?¹H/+Æë?Ûã¦[Q'ø?¸ÄOh²–ÍMIXED4FGL J1724.7-3737?¨Öåác¿ð¿Ï"èbUÀ9L‡?$>À:Îr«G@O²{<â4@YH;4Ž?ÎqUää?Þú™#R @
.9™~Á§@rx¨ˆIæ¿ïâ7,¼÷m?=î"2¿çù҉¥/пèsGà¿Gÿ¿ç!ßMØÑ¿ïÿè2_NUNASNone
?ӊݴPª?Ä?÷S€}
?´ºÖ‹ÂŠa?­nÞɾ>X?ã£6T¿Ž»?ŘÊÀò½¼?ÏnK{î'?ÁUý‹d*U?¹'ÏM-ü?±îd*~K?åbÓE'?ÀQ´υÔ?Ó!ÜØ1§?±Sù""u0?Àž:C®ç›?§$P1êµu?âGƒg(-F?³",uø×L?Ðle'>?£ÍA;ß,?ÃÁ8àØX­?œûØ9Mº¯?âÙÊÅ?§Bfw›Q‡?ȞºUPêS?¾ïìGͅ@?³}­
–uá?¬£ç'€2±?çh›È¦€?ÁDÆn
ú•?¶–Á5ày·?´V4žR?Ã%@8KÃD?À‹o#=?èc×Êú8?ÁóIû?ŘùÖÆß?§5¼#­_?Á†ü¶ó?ªÞƒb{?æ8\Èû(?±]‹^Ëðâ?·r­Œ¡«º?—'HÓ׊?ËŽF^?«·ý'?æLÆÌÏôA?®Ö¬]aG'OTHER4FGL J1725.1-1924?èwj¼SG@"ˆP›ùÆÀ9Oç"!°TÀ;‹M@$³>@FíùXŒ@_ž£Ä•Ç?½uQçÿƒ?Ê⬩@3ٛè(s@@~æ?ïýüºÑ!Æ¿á'Ñß^¿â7Š`@²x¿äè‰÷e&Ë¿î鱿«&4?ÚD¾@BoUNASNone?ÕÌþùù3f?À5)¢»¬>?«K8S&Å?ªÙS9€,Ë?ãgûϙ°Á?Á4›JDW?ÝξÆ"'?˶T^뷍?Ì¿3nÊí?Ä<Õ*`É?ÓÒ`§'ø?Ä1²p]¿?ãÑW]Mt?°*YciHþ?ºö)<Rn?£wÉÀFå>?џǤ!|?­þq?ä)Û¼\oË?£®ºÌ›ÙÎ?ÁbËÙª"?™à¼ÊŸl?ÍöŽB´–±?açTº!?ÃÖl	^?´6ý}zÇJ?ÁÛ+'~§®?»
[}Õ?據/ÛS½?Á¯×&J ?Î='%¼ZÂ?È´x ®>?Õ$®àþˆ?ÊÏüç
ªm?ÛÇG¾@Ô?Ê>k|$ˆ?ÚðÐ.£y?²§Òr¢?ÅÀË»ïs°?«X­å,ÊK?Û
©QÙ¢¯?±Ö¿#ö&?Õ~Pèйk?§Ë+JÒ#]?Ïû¤=XóY?©¼9ê·?ڃÜù•­§?¨2–̓ÎNMIXED4FGL J1725.5+0840?í\}V9iû@7t>–=ÅÀ:8"ïïÄÀ;ø³ÓÃt@o‡]s@®^L¼q?Âv'ƒzÉJ?·4—¡Ç»k?ðÃmrÊ!ø?ûF°¨ÿ¾¿æáÀå7ý¿ß©jÝn…š¿ë¢†ÝÕ2Í¿àÀœ2#i¿ïýR¦–_¿ÝŠºC2YÄUNASNone?îø…ïÝb?—jý¶
?~–šó7Ô?}{Ô‹A{?™Yˆ‡x"Ì?"_åf:‹?TÒ{?¡²
21oS?'nßòôr¼?•§Üð‰Ôû?š ½À¹oØ?'|Æ}'öï?ìPՕÇ?¤:£!Õ(@?¢<á7	V?—³ï<UŸ-?´Zâ½ ´?Ÿ©Jðäì?íÛ
/âN?l}È? ­o{˜9¹?'|í–7æ©?®Tßß±Óc?‡GrL?íæbÎ4¤?£ÖbÝ Ö/?"p¿4ý›s?ø¡Ww7?§asƒøv?Ÿ¾pÿ̝`?ëý¶À¾?¹¨Mˆì?ªþŠ"òâû?±µìçۂ-?²—ü׆®?¨U@ÙvïÅ?éaøjVØK?®îœOqü?°|º$ˆ?¡—ŸÆéºÂ?Â:yÄ?§ìmêÓÃÃ?è$oü<Q?¨=osÁä?¸JøEҀ? šÑútù?ÃHÄ	YÅï?¡s"ÕÃ+AGN4FGL J1726.2-2903?ë«ô«õ"@'cj2¤À:3±6nQÀ;x'æÏ­R@Œz@ÎÀ§¨?ÒD@ ×f?ܺé"Ä@	Yšäó4@e
˜ÄÝj?ﶋ!±«‰¿äÑï¡c¿ÁáBWC¿äµüŸ|2¿ïýX «Ó¿ì òʍWUNASNone?ÍØݖ‹?»ñ)«þ~©?±œQè|—?¥'Ä©‹ÖÃ?敖>41û?¿'i@د¦?ۜÁ:}2?ÄqQÚp×â?º&ÁµÂo&?°‰¼j´<?ÝَgÇÃ?ÂËâ4Eµt?תWóÃý?²+>#ßÖ?½eåè<ü?£ÙtҚ)'?à~e!lâ?³:ïÓ؜É?×é}HK"?¤dZpÚu¼?¾Ø6¼™g´?˜æBÈ/6Ø?à0:™È­G?¦Ë瘬¿?·ÌIˆì?¨ ç¢9q?¾Ôñg"
?³xõ§dó?é+Ø¢‡Ã?¸éºAU?Ç }%<?Áµ‰àÐ %?ı9|46?Àjµ€í ?äë'X:\P?Åë,*Î?ÉY~L2?«ñÉ2Fa?Á»ÁÏ:1Ì?¨môï
ù?å:¨-8Ðà?³-\GfŒ?ÃMJo©Ÿæ?ŸäÚü¦L?Þký÷_?§·MûÎ?æˆuÉ/?«eNÓì‰}OTHER4FGL J1726.7-3930¿î·Ïæq–ÀVq¬ÆaÀ9ÔÙb…UÀ;>"à4ê@>=I·™@¶
~C›?ÑkøvžÂÎ?×(Õ_°@Œq'êS@ØéÆW½¬¿îo<c]j?ïÓpöa7¿åƞµbLü¿èÕ·UlC¿æ¶9­ ·›¿éàbiªUNASNone?æÑX¼s}?¾ÖLÛÙb»?ü£}P?wè?N\tï?Ó6|ñ9µü?¾'.*hg?Ûuíe&S?ÆàÀ@? £I\õŒO?ž¸#øÉ#?á;?sTØÂ?Åq²8»¢?â5h¨=©â?±æñ¥W›?®~°Ü— 9?˜Âݲ8§?×ÅX"–¥s?±¤@"³8?àÇ-¶Z?¤ŸpÙh÷?®ëzzAF?‹	4ÛIªS?ڔ5RXx£?£Ún>)¹ë?ÙBËãTý?¿àÓÙ 3«?"ˆÞ‹f%#?Šà Q`?âºSúÊX?ÀK€à]?Æ혖±ª?¼-• ?§wtªÇ Z?ª¢1¨–e?éÍO  ?¾)c.V2D?ÓO-èσ?±32ìÃ5•?µqÑó?ž#ÈJö¸?ã´¹)E¸`?²"÷ñÊ¥?ÐDõíf?¤ïÐmLPê?¶Œ®³±z?_Zi?å&GÃ@ºŽ?¨z%x1MIXED4FGL J1726.8-2659?ÓjçÛع@$ý£.mÒÀ9º`@²w·À;_œÈù@Bm¬@<eü´%?È÷ùñÉ?¶éÀ£s¸	?ós̀v²å@ýb–Î
?ïÿr ®Ì1¿Ý§š
\à¿ë'ÑÀ§zƒ¿Ùµ'm¿è1B}Sö¿ïÿÿ&¦³UNASNone?Õ^½c£>?Óª÷Ád†?Ø óÝCú?ÞY"A"É?ҁf/ù‡?ÑàHæ?æL'Žv?¿ žtärJ?"]ܲð?"¥pŒ[Î?Ò!àfó"?¼âw]HtR?äŠU¬.ò‡?²§Œ&Š!?¨+)›Ò%?™£eO""?ÓêOBø
?±ß5ôÈX8?åÊx™Ä·ª?§•äð¬'?"6Ý»D`?qEÿ¼ÙÒ©?Ó7 ðûÖ%?§O€Ôf?Β‡t±‹[?IJmÈQà?®ÛK›­ò¡?ÃTÝ잓?æm©h?ÈÇÅwÃÜ?ÛG;;H5?Ãú'ٍÐc?¡u—•g?¤@Èþÿ'}?áEñýD?Âùñdü?Øæpf3T…?³MæýJz?µs\¸i?¢7¯sêk@?àì™jí@?³ò$Y?{/?Ú5¯?±w\=N²C?¢¡bÉujÀ?‡e^ ì–Ž?á»"Q¨X?±Ù¸Ð¢MIXED4FGL J1727.4+0326?ÝGn=B'@4:GýœÀ:5N`¶#=À<§Š$Ô@˜ŸBÐà@ —ºœH¡?ÄOI¿;¿Ÿ?њIâøc@V1µ"±«?ùÝ£í¥¬¿ïÿÿ>¹ú?ïÿúŒ—Ó¿ÕÜýë©¿è€#¦Î6¿ã(Hr_™¿ïöÈHٍ¥UNASNone?ì"͑\£?¾ú¸ñý?Ù•ë¶³5?‹ßR
&?».`·6Ú?½Û.ˀ­¡?éîH²÷8±?Â(OZíG¨?¿÷Fƒ½?¿-ÚëAØ?°–tSÂ}q?¥‡‹báò?ê7Yº?«œCÂøb¨?§'Ï_4?šÏ×Rí?ÁB
œµ?§XqꪸŽ?æByFèǪ? ¥ÿôæs?·é»ÅéY?ž÷Iä×?Ä>1(–÷ÿ?—Ük®ØM½?éY:«ˆÁ?Âͱc:|?ªyý"ÿ).?¥RÄ׶?Ãý3Ì$3?ÁóLuEô£?â¹ÿ~ŒH?Ìò–"]s?ÒJ7=¦K%?Ë4²S.?Àƒ"ŠƒH—?´R\>"eW?æ"G¹ìº?±÷a"dÛ?µµTXxõ?¡Ã‰T˜Ã?Ë6ìƒÔê?¯4)tºß\?ÜåŠ"†?«/ÔaÊ(?ÐL9ôäè?±Nåf,Ìë?ÒÎF°¤´;?«~Ð8¾ÃAGN4FGL J1727.6-2304¿î3=͞Œ@37ÿJÎZÀ9O¹ã»ü›À;O¹ïzv¿@åªi @hLŸëÃ2?¿šâÑF?Â½é:ø@€¬:†
Ì?ÿ¥ì©&¥?ïò'íÓ­'¿ç5÷¼d ¿âµ{A¿½ñ¿ä} ½ê¿ãG ñO´¿ïü&Å¢·UNASNone2FGL J1727.8-2308?ä)u'@_?º¬—ï$?Šw~ù?€ú5™G—Í?ÖÙYú¡+?º•ò
V³I?ÞoÞ)–|Y?Äeqb²–…?±½"l"d?¨‡¢9:=?Ý ¼»)-Ã?ÂeÚK%1?æ[(ü^Æñ?¯¼[Úʦ?¢xvϹ=?"ŽÒz½‰¯?ÐúŸ-'D=?®4œ% \?ÛÚæ&KTx?¢"þÇÝ?´IqgÓ!E?Œ!`ӊ?ß½~ÈX?¢Li"]ˆ?ؒJfE?¼ÑUï1ø?«'a^bã"?¡—ëNo?âdܬ…?¾­(['¡?È^Áp$?½©9Ž…Ù?¿B"ìdm?º²k&Œç?æ
'wÉ?ÀÙƒE¢Õ?Þ%IçÙ"?³qwñ¬•?¯Ú;+lmÑ?™ôEàא?Ýßn³oŒ3?³³4X?ÆÒ9¢|Ûã?žªeåŽÅ?¿3¯?Nç<Zœ?æiK öÖÈ?¤i¡Q›iƒMIXED4FGL J1727.6-0849¿é›Ð·×¶ú@,LÃ\á'fÀ:=LÖrgüÀ;€S`'@ø%ËÁ‰ù@£Ho›?ã/`•Áô?âræ§if@
D7'MLº?ýÔ(ì]`Ù?î'—L¸?¿Óx™q¤ˆ¿åëi~J‰¿çžb¿ïûh÷:^¡¿íòá~µ'žUNASNone3FGL J1729.9-0859?ÜGÅ1ßq?ÆàíQ'?³íxÈK…P?­€\çϗ?޼ܛ21<?ǽȭ®N‡?ä©ÌYh?Íü	®Þ?ÉóЍå~?ÇØ;Í­ê¬?ÃgðÆzs?ÀÄÊ[³!?߯qO×s?²¹¦ú12H?»òºi•<_?¢×—˜Aèž?ÙSàÃ¥v?±öÀ^¡?и=ÍIí?¥""'bY
?ÍiKçÐ?°ò–fÁ?àIŽ}Ëv¥?¯"õl`øÕ?Ñ}ßm¨ó?¿î´#﯌?Ÿúdh=	?¸d•d'jç?♯ˆvå?Åq¡ØØI?ÖbځQŠr?Ѓð	Fê?ÚÓÒŠP¦?ÑHN †+?͒¦ÖnK?Æ	ƒùìŒþ?ת Ô¥£?±Ó"ý}Á?Ãa|*⛅?©]…ŸÅ5\?Þ¥!ûïû?²?Á!
 F?¶ÂöG5å?žTéBL¡[?ÉÇb_p¨à?ÁEBgñg?æµÈŸt,«?Àho?¨âbMIXED4FGL J1727.7-3621?ﺢ/ë*0¿êƒ©8sÀ8éXjËPÀ:6&æô–?@ 2¡'âE@j r}Ì?ù2«¹VÎC?Ô2k€³š@fî0Ê£'@ÜW·L?ïþÝ@7}›?Í.-ºÎG¡¿è¹]"?•A¿äÀåÙ
Lð¿ïÎ¿ìº?äŒt¸8ÁUNASNone?È×J‰æô?Ãåt%8@0?¹.S7{?ŐªIa•>?æšG'ÌÜù?Ë-¨´•J?ÑLº÷@?Ån«>n?³SkõÛ?µ¶Ÿ*P:?è±L	² ?ŏFöDÑ|?ÊqÄnëT?®¯jŸμ?Êo³Y?°8G€ÿ?âÇÌ÷ƒÉh?³¼yÅù$î?½'?à?ªµíKb?¢&Vªuy?¦ª×iàŽ?ë8»Òmdv?±A	טy?Á+[
º0?¾vbP	á3?¸¯ ¦…?Â8)(åžÍ?è±s+µB?ȋͺ…ß?³ål/ ?»ÁÓù«–á?½_%e¦^4?ÁËá)?é×x%ÅPF?Ä'jv°$d?Á绣ã'5?§´|'n´?Í0þ1ºH?²UԐ¸?ä9ї"8?´1­'˜ö?ªçŸ]"4õ?«¢gŠªs?¢8¾ua¥
?·^n÷Ôs?í-ú"µ%€?º(!¤P¾OTHER4FGL J1727.7-4041¿ê_Kg¡>À	ë9\B 6À:B–Ù˸ÑÀ;Š¶ÂŸLa@'KåÓª@yX`ê%£?ȈH8}õÏ?§[Õ=߉"?ãè"=ƒH@2Âô†Ð?Óì{¿¿éòH‡XNv¿èÁ'ïV¿å'ˆ˜ÀUÆ¿è"Æ@–ž?º3˜ôUNASNone?Õ¦B—ݵ[?¾U-)¿þ?ky¢Ÿ!üÔ?_ÝX+°?åeÉùU?¾nLÊð?ãˊÏ!?ÄTžŒaf'?…¤³ô¦¿ú?ŒÄhðÇb\?Ù%CLl%~?ÃÉôϺÜ?âÀóÛY'}?²|&Ò]͔?"ìÚ\£9?†:Œ
¬öJ?Ù/J£ð¾!?²s'º47Î?æ|gY!ü¡?¢Ê[Hõ?‹ŸÕK`!?k'ôDþO?Ò/,O¶˜û?¢‹ØñVÐ?ÇU—	$¡?¶ÕßؔÂ?wRՅ›}?p3™‹ˆ!?éûô'¹€•?·ªI©½	?Ò܍ñ+.?Ã͋èÅÀƒ?‡t¹z‰ð?"y>ï`U?æ3æ!&1?í$Ð¶M?Ô×F)ýKè?²C8l®"?Ÿ ¦ò%T?ŒÕ˜1ì_…?ä›W³+w8?²‰ØënB?×¾#裩#?¬0¼'ʱ?™Û"ýSú?†§*j¦?ãRãµÐ?¬o…E>MIXED4FGL J1728.0-3550?îV:ŠH ‰¿âÅuà¬ÓˆÀ8]qHA¸1À9óÍêÙþ@,³ô8Ìz@‰µ/ê©?ǃԠ֤½?Ù°ì1"@ªàéºC?ý­¼ÌN¢¥?ïùÐfqN¿Û™¨G²F9¿ãpöBˆ¿éÌòŒyöf¿ídÚu+ü¿Õ£ãßãÕÓUNASNone?—Ý€]ºC©?–Á%¢òuã?‹|PÞiØ6?¢µ w‰?îÓ"¹ŠÈ?žJŽí¹Ä?ÃE¶œÎq,?¾çmH>?ėžëp¯s?µCM;Ïà?檝ð7Ø?¾PÈ/M½?¹g@¥{hñ?¤»ÕÝRè?¹ýÀ'Öf\?£ª'Ìa;0?é"_æ
ç?­i5$Å?™£ttŸ?€t³N€$€?Á©(Z¬n? ˆÞ<_"?êșe°ø ?£1cþ–Ä3?ƒ³C¿ís:?€å¹Žq¿U?'x¹£oô>?"«¹µ=?ï%m$%i?˜4Á÷³_¦?¤ºæ›U–?¨3üÑIl?È}¼Ä?¿b6DÏV¯?谎"+@v?ÀW•Š¯?°ô}=]ýŽ?šŠ¤x¿?¹´Z$¹Æ?£—FæÀÕ"?êªåôU?¨îÛ"9—?yx¡¼öo?e§áÒ¿N?Æ·ÁÍÀ=?¬MÈ×<î?êF Í.`T?­eoã–'OTHER4FGL J1728.8-5131?ï_ ªº~À"\ú¬ÙèÀ:•:a%À;ñ3eˆ@'hC¶86@¯n'"šV?Ũ%$&Ñ?ƒEÍê"Ò?ÀÇ?EvW?ÿfwM"]p?ïCE.Þ9Ý¿è¼ýÇ%C¿æì€üê¡Ê¿å)	
Å»a¿à[BEÈa¿Û|M"ȁäUNASNone?è÷ªÞ"Ç?¿{Ù»?rÚäw\Ï?eç†v!%‡?ˊ€a<?¿3cq-Y?èƒÛF¸ B?ÀnÉKãÙ.?w\|è?'øe<$àh?Í5¯Þޕ?ÀҖÿû?ìh™‰ñ.?¡Ÿ¸hM¢?Ô¥-ÖbÝ?sƒ®¿©JR?º€Ÿ•¾2?¡Ó
yRa?í֓VxK…?"ô¼›uh—?rP£&¥L&?T[1ü¿À2?°&[áj—?"Wò–q,N?âV]O™ùÄ?Ç)°R˜©/?|¬tœBîø?oˉÌ_#-?Úà"Ž<Ä,?Ç1€ûw?áÈö4`k?ȵÍ4"I¯?|³"Ú[ä?‰!`õN¦?ÛûGà¼v?ȑ݇¾?ç9v'à^?°¶Ëi³?'@:䟪¿?€~à»®Å?ÐiGÔ]˜?°="N÷?隟þÚÞ? Ó!0Äqs?‰ZÚFPÿô?u ÛÏÖ/?È3ݎLE? nmï7TAGN4FGL J1729.0+6103¿àVÐ;
¿~@@³¥ 8LÀ;H!ÔfBÀ<•>zW@moe©P@³ê-/ãó?ÕÈ˒:*?Њ+<™¹O?÷åþFÂ\1@	0=Wyc™¿êë?{@¿èb¼Õ"p¿ãÊHŽK¿èìóþê×$¿ïÕ»Ÿíq¿ðUNASNone?ïÚÉ%è
Û?m´	/Ê?\èµï/f?%׈›"8?fÂhMç?]˜ëƒP•?ïšç$;ôx?'½Åª ?cRæ&i?k¯ÉВ+?"q}sƒ½]?|1=(AJ?ï%?IìÞ?yo‡Á7À?{ç+®"«‹?~›"L?"^K×ó04?‰j£T0î?ï?Ïò#Ñõ?w"<`Úg?kÒTÔ¡5"?R‡°àswæ?"‹·¦Æ?vÉP™àO?ï~–óEï?¨ôÈê?#?~9EÛÔ??¨¸X$?=¼¡úòÀ?}ÝÕv}*?îéô«8'?Ç"æJQ|?u¶¦ÿ¸yZ?'	uRõÕ?SÀßh6É?˜'ºrÑ/'?$éæ°?•ºR<[ýŒ?"BÆ^2?"¿9µ?¢5
ƒ#¦ò?'¥n¼˜?í¦ž‹'ö?˜£Ÿfià?}ñd0n?svð˜ø°?°ëõa4†?˜r|³Õ'	AGN4FGL J1729.1-3503?Ý‹pa¿Õ_/:€.À8Ý6ñLÀ:XoÌW@Š
Zvï@QÛèº?Ç¥ÿX:?Õûò•í=@Ç7ƒ$O@ƒê÷Ûj?çÀ;Yrb?Ô¹¥¨›•¿âŠèü®<¿ÞÛ	í¿Œ¿ïk›Äí{¿ðUNASNone?É­"?šQkðxl?¢bŽã¯¨ª?¥Öà6Œ.?îb²ýW-?¬ÖL‰%?¾K<qþӎ?¹Ã䨮ü?ÓüÝÇØ?¶I¤Ê{ï?çQ™:N/Ž?¾Ë+À€Áº?¿8J£Ô?§ð:_(WÙ?́@©¶?®:TÊ
©?åµK?³8?°Öȯv!?¬Ç$v"ÍP?'
ÌP¸ð›?¼KÝIØÍG?ŸÒû©Šý?êªwb?¦ZÉoã!T?šw]n"?» ÂLHá?§¶cÿj¹?©ÈTB!™?í°Þã¶ÚX?½u´œv»?¡bҌn&¾? qý¯~ïZ?Ăf=1õØ?½ö?LqÎ?éÉ9G§çï?½¡Á"Ð÷?¶‰X®Â˗?¡ø3c÷Ϛ?Τ,5¤7é?°øÇ3}'j?å…Éܾ˜"?²Kü´šG?"}kËêŸ?ÛtJ¡¯(?ÀzŸ>°P&?¬AŠšëVº?ë=k­	?¯<…øOTHER4FGL J1729.2-2509?Ô-Ÿd@^øÀ9â"Óa;"À;3Ï`ûÃ@!/z–õ@uýfȌ?Õ6»©?å)Á¿þ]>@CEÎ@j?û_ò+V?ïÿTsõ›"¿ádpݸ­[¿æ}Kà~/†¿ë™ðlF¿ìV¯°¿ïÿÿ)@k*UNASNone?۔ê+L?Æê}ŽîgI?·"í¼2U%?Á¨/xWn?ކ©§Ù£J?dzöù4?ÑÅ3–/Î?ÄíÿÆãîk?́ÍĈI?Âb‡ÿ¾;º?ßù刟:1?Áh駽¸w?ÛTË/$?²ù5—ñ¶­?Á\>Å7­?¨šüÇƐŽ?Û䆱yN?³"$­÷Y?ÁÝ'Õ&°?•×@qžÎ™?ÔS¸ßZ$?¦Í{XÇ߁?á^ÜkªB?¦öâùH§?Êw—*ow?À,ÓVÈS?ÃÉӝ8?à þ)ˆ†ï?äo؀'À?È^CF¦?¶Àið$8ñ?´ýëTï'í?ÕÖ%{Pó?É#SâUJ4?â<à7°ø?ÆYmXÃ]?Ð(ƒœ­]?±
U'j?È@"ªt2W?±õי­±A?á۝c¼?¶-d:ßÙ?¡ÌÚUúÈ?'êJ4wC?×HQ¨i@5?²×ª´§š—?ã?	†<Æ?²P°ZpüÒOTHER4FGL J1729.4-2831?îŽ0Ä1âj@	È*ÜLœ'À9¸ª½®KØÀ;_ÐJ/Ï@-ò»ô¸N@m.#(ú?ϝúé×?âÛÛÈé~@‰Æ×p•?óëà;§R?ïÐ•¯)N¿ÙsÇwù5á¿æ(oÀ';¯¿ì6ĸ+U¿æÑôSúS¿ïäîâKd,UNASNone3FGL J1729.5-2824?É©óEm"?ÁÛ׿ø†˜?ƪö±v?Æü©S æë?ãêÅ´æ¸B?ÉRŸP#=?кlº?ʞW³'?ÍE ÍYSr?Åûê&ç?àQ"Á›ôÆ?Ç>®HÊ?Ôh²Kþ?²=÷¥ßT?Âýþs
?ªt§"¯K?áFxû‡?³T"Ü	o"?°Ùþì2,s?‹GoF`Ð?Ñݍ,pá?©0ðÁ|??äõùŒ…!?©î(Ãã?À¢'¸1?³‰!FK¿?»Î׏¯œ!?½#¤¸#Y?è])œ°?Á'Áš­&?µŒÉªíú¦?½›ËÒ?Â'?Ó¸yJ¼Q?Ê÷ñ´È–?ãr*%²0?ÊNߌ%?ÈA®>IðB?ªÚ#s¹?ÂUŽûß?­º¿
Ç?åZLÌ®¼8?³·&›•à6?£@õ4?t÷Hà:[$?ӖÁ¾âåy?³Ͻ†Í~?密–e:J?³†moKåOTHER4FGL J1729.4-2646¿ÊqNnDx¢@¬¨ââ¸ÇÀ:`{l‡è—À;ˆÌ&°n@û8|É)T?öœøä'Ëø?ç§"ïQ0?꡵A•Ì…@Ãà{Ö:?üôRÝÊ?ïÿð懈ö¿ë$¦=¿…ãÑZÞ¿å_ú†C{¿ïÿŸB%‹¿ïh‹9"†UNASNone?™ürޘ? Lcí։?X1Ã:2œ?‰½ñv?î껡Åü¾?¢ú+mT?߆èw"KY?ÍÖ«a±å…?µ«|÷>ã?¶'¥1¦‹Ý?Û8hnN?É^ka31í?Õ£KSíñ?°jG8Ò?Åfß-ޛ½?¨]'ñ‰à?ß©EV©ãq?±wkñ¶S?Ï츋³c?¸Ó¢étY`?žÀ'a)N?šM?i…!?çF>ቕ?½T3!Ú4?ŽJº…ÄÇè?'APohŸ?†Žåx¤³Q?‰ô"À§L ?ï,™ÝÃ?™}'€_[¼?ІOÒr ~?Ì`ñ|¯~?À÷½'ŠE?ÂùÞ=bŒ?ã~ô'bM0?Ë÷·¼ÅBÀ?Ð<œc"!?­Åp2Ô#ê?ÇcÇ v©;?ªçôsyÙ?âÀQ!?°â#§‹0?Ã÷txc¡?·½¢H7þÔ?‹ÎS;9³?œj´Á͜)?ê'ê È7?º…ÁyÌ8—MIXED4FGL J1729.7-4242?ß4ÂcÙÀ–Â&€IÀ:71xH:À;£¨z-@&‰/=õ@Q¨òÓ?ÔòI~N9Ÿ?äh¿µ<@‰å\ËO@íõ!È}?íD¹ØÔB?׸ÎG*a¿æœ†é"¬ñ¿é‹@•¿ïKtÝøn;¿îÁ†b…0VUNASNone?竎áÚ¥þ?ÂĚy=ƒ™?ÀËrD@ ×?¹Õ¹ÒÁz×?À†R4UG/?¹qJ»¨Ä?ÑÙÞ*¾¬?ă
²œ±?ÈnÈæõS:?Àj±#Îç.?à÷^±;KÛ?Ãøæ?SkÒ?à'`ò±?³Áã¬ç?ëûÆàNµ?ªÈï/"?ÕÛÍ\OóD?±™YÜ)?Э.T"Å?¦²3¹'ï×?ßÏp¯Ú<'?²*ús†Ý?Ðâ!Ñ>ª?±-^q2Cà?ݼ¼°R?ÆC|
2?Бbwˆ;'?ÂА?9?ѱàØrrc?ÃS[‰`õ?»'€tÉDq?»ÞBÒÖ?Òh~Í)Ë?Èè&§V(?ãYŠÚŒ?Éf%¥ùEÉ?ÒùïìGͅ?±uÎ9l?ËÅx/;¬Ô?±ì*Ù²\?ß#Sý-<Ï?³Ú&PÇyÄ?­a»¢Q$ë?"­¶²GÞ?䮖¡?½jn'`Ø?ÒöœNª²ò?¼vM­:"ØMIXED4FGL J1729.9-4148¿Ð¯9.òBÀºG²À9t(<æÀ;g
"fy²@àn"0žÙ@՟Ú%{?Àu	l?·uPdˆr?ñ>³nW@Ç'¹ØSi¿ï·б]Û?ïÿ´Jõǘ¿ækÑ	ro‰¿æ'á>sÙ¿ànw¬ßÇ¿íBåøí½UNASNone1FGL J1729.8-4148?ìc×Æ®ƒ>?­i§Ý'?q¬Bb)?g¯ÿ
h~?»Ð7ô³=?­8­MY
Þ?êMÇ-Ñt|?º 7¥U1?i&d
à¯(?pq''\ð?ÆdI¸}+ò?¹»ÑoýF›?êž…ø¹ ?©«%¨Éï?™ä
^±D?,'qa¬?ľIfÑEW?§._.§?룜׌?'AæFžßz?'Nç›d‡Ú?r¢æôêê?¾OeÕ6¢?ë]pCk?叴¡ª,?¾³î?ÊVŒ?'Ežîã»
?‰P´➿?Ó͖¨ÅÓ×?¾¢ÉÄÐo?âH¥RàL±?ÇùÕ#]}4?|†m²šÐ?‰åC"-Ô?ÚüTº'?Ç°€¹¬g/?á1
‰ºÿ?µV4†m¸'?°Y3o£d?Ÿå̇ï?ه 'õ$I?´4h¢IÏ)?æFã‰|Àñ?¥œJ¹l?¥ï¥("Óú?ÉfÜpi?дDHa÷?¤¼G‹³;§AGN4FGL J1730.1-4343?ï'¨æiÀ[ÞM'ÑÀ:.¼ÆÅKÏÀ;¡=ȸk@ª|ÂqU@S°ÄXŠ?Ñ°™É=v?é(¶!å'ü@^(}ˆÂ@¸¢kOYZ?è–Dzƒ?í`ov°`…¿åú´f¤z¿ïý»aëW|¿ïí¼ '+"?ïƒnI‰¶ÎUNASNone?ÙQ"Sxg?ÉÛ$"
?¼^Él£Ÿà?¶*ˆtA?ߖ‹ƒŸ¡?ÊE¸Äúh?Ô²½¡W(?Éٝ¸´?ËÓÒ…?Ãæšmõ.?Ýc¸fG?ƓÇ÷¿®p?ÞiÕ
!Û·?²thõœUµ?È8½—Z
?­¡oÍ~‰¯?ÕyÌq–†?°t¹=ulÄ?Ó?£b´ïÐ?¬z†›‰Y?Ü¿÷r£òŸ?²™¾Z'ŕ?Ðe*§'?«
IT
NJ?̚tAè¥?Ã@%EEÃ?À·'/<%?º––&iî~?䫂c¶Ív?ÇebÝgF-?¿d†Z€1Ç?Á3WKÒw˜?֓Ïæ1Í­?̶•¾BÆN?àɇA—ð?ÌÛÒcºˆ?Ò[å´ORy?°Y×ÅÕ?Ð&¯òvŽ?³a(ùnL?Ý}jY:-ù?´gñíøÔX?´Ð5
Þ"?›6·–¡S?ãU s±O?ºƒÙ
j3?ÔO‹?ú?·'l¢oÊ÷MIXED4FGL J1730.3-2913?ïzÒ>Ú8ú@Z¡ô±îÀ:Àk<ŽüˆÀ<Y<Íù@Ã÷h+ã^?ÿ{xFbºà?Ö·Tà¬þ{?ïÿp=½P@¶WuÇ,@‰-Vû9r¿ïa.ƒ¡	Ð?ïì­"šB?¨o‹þüIè¿Ó¼_vÞ¿ïÿÿ>¹ú?ï߯BxJ"UNASNone?×t!ÝAÜf?Ég¨ô˜]?ÝHpS?̔$k*š?Æû«´›Ÿû?¿UݓTÂ5?Íyâ‹G˜?ÊÁÅZ›4­?ՈŽK^?ÉNôW³Î­?Ûº€¬/?Ö?Ê澚¨?áLºÓuÅ?´6KÂ.?ËD¿àÞ°-?¯1t._•»?ψXù:>?±õ{9(¸?ãtÄÅcÄB?±ÚRÖÃnö?Ð`INܽ?°úN*Á†?ÁlZNޒû?¢û9ž;¨?Ñ-\ª%?ǐó,Ýُ?àÙ«ãF7?ÎÔ¯Àޓ/?Ê>—!w?ÃMLëQXs?¹[·ñ$n??ÀC¸¢¯~?Ýÿö
?Ð?±DÊÏ?Û©öñ/úç?ÎށÓÝÀÄ?Ø=ª|»?´¸7§Q·/?ѽ¹ý5B?´ÂÁt€º¸?ÖœUûN?µéšfÊĝ?Ômõ¯w¯í?¶	ÆФì¶?ۍËlqå˜?¾¤Âì½ó?Ð>å)K9?µK·å§<¯MIXED4FGL J1730.4-0359?ä-íaþÞÔ@/ý™gD²·À9¡ƒJ¢»À<	²öañ@ûŸZMÔI?þ´zuçãª?À_©]ÜÕ?áp'S­Q@B¸A$~?ô˜0m±v¿ï´qV"q?ïÿÔač¿Ãݨè)b¿æ¶ã¡¥¯¿ì´/GhG¿ïÿûÞ]BüUNASNone3FGL J1730.6-0357?ž®Däpz?£*Í¢Ïg ?îld4æo?´=Ë(Î?žä.–ª÷œ?¯Mž«g§x?žîw¸?£Ü$á9U?í?´²
?±ºþþí;?¯_ÐA˜É?ª!äé9š?µbê°un»?¤"wß?é©Óã…?­™S7ZkN?½T¶-¡?¥åƒwÐ8?±órŽ¶é@?Ž¡Qr?é:F9ÜV?£Ú^ðK8*?ÂýŸ† I?Ÿü)¯òcš?Œ¹À²`…"?Ž'yyÜ?îÑÀå7ý?£œ'´CÍ?—k‡×Š?œ|ÆO£–?VÎM·`?™Ü¥­°;?íÍþ
¬1?±/>Gj?«J™:Õè?­)ê«¢30?¦T•U'©Ü?›/cô/âþ?ëi'š%†?©ŒL@Ûñ?¹‰$™våä?¤Wس¡?Æ	lÃÖ7?'³.s¹hÊ?éゥ{?¬éù…÷Ø?Ĺ4<{9?ªz‹‹‰Â~PSR4FGL J1730.5+6018?×ñ v'"C@@¡êhìSÀ:ǀõ]åŽÀ<g;.ª7@:ê¡tˆ@øåY‹?Ì<"1/?Ç£&
UÄX?ùÐéÅ@X—)§Ä*?àℏFY¿ÏRôčŽ¿éo6žø~+¿ãWB\	¿î{bâMg'¿ðUNASNone?ïO¹³s?……ü{·?')×k>™?urÇ1}1¡?‹'±2í?}¦6¥Îo0?ïtk.Íÿ?"2;µço?qõ­3ô?pùeÌ(ˆC?‰ê]®í?|D̓mÁ?ïZqvËõ?‰7MQÕP?MÀË2S?¬UyÕ<1?•-Ñq·½?'il]|Ú?îÅ+9$õê?uod?'DJ—C?jóÕÙr˜ë?–NËêúŠ?nÞËan®)?îºøºøu-?"8åÌ9?[€•wÝ?‡ž"e<?˜Ehé7?ŒŒ&pUs<?qxé ? ÄZH²?†h#¦1?Šr)õ?¢=€%?¯·?˜H²Õ2?îI€Ûc?—M¥Žë è?'`f	XË?‰±Áå…XÚ?¦k4ëïA?¼V¥+²±?ì:žr­ƒ?'eKÀ?§»øKþ©?ˆÞNµ•…?°.äEĘ?Š—¼eDªAGN4FGL J1730.8-3806?Óäÿk÷~À'¢&0À:@[9âzÀ;šÒרÈâ@LR_žK/@@þ¥Œìã?Ñcêöƒ|?㎻ßê‹Ð@ÊeI/ôº@AæŽÿf?Äöë¿Ý—Š ­_¿Ô«ÉGNÏ¿ãÀ'¢Ü8¿í"rmÛ¥®¿Ý#ÌbïŽnUNASNone?³<ȶ§AY?¤¤¬†×?Ѝ'H¡âò?À°Ü
Sòé?åQÓD¾©|?Á˜+E?ÐKƒá÷Vc?Á¬Tõ¶â?·Ý>»ÐÇ?­š‹ì\d?äùÂfõàö?Á¡âaù3!?ͦô–?r?­{Ç«Ô?Ò<"m,J®?±¦çÿ·?ÞïñG³üO?³·çm?ԋÅÍ÷f¡? kl­ÏÇÙ?ÅMì†g?šÎïh—¿?àf¢¬#N?¤‰Mïg¥'?¡Ð
‰¡v?'\‹{õ?ςE†IB?ÁÚ?u¥]?çmÍ&Ә?Â).D…¹?´JؙÉ:?¯É£Á)?»KþtÿJ<?µ"鋼?êvÖ1`±?ºS7#qü?¼1äԀu[?¡Ò
i'(?ÔÙkd/²ÿ?·ú&/ì62?â

³XÕ?¸V[Vgì?¿5áVz=¼?—C¤•W1î?Çà]wKÞ?§ÏÒXÛl?æ!>ýÒåQ?«KÅB˜?¢OTHER4FGL J1730.8-1123?émËxÉQ@(EºÓ¦âÀ:´Ÿèh3ÆÀ<†íÅjÙ@!OµX«h?ú‡ºt´›?ÕD[å$x?ÎJ>ýìªc?ñL <K	ê?ÿvà.~m™¿ìhûl‰?ïø ÅÝÅC¿æN'à¿±kØ@Ho…¿ä¸
¾
¿Ùj"‡0áIUNASNone?ï€q2$ô?˜¢¯Æ@f"?a'	´yŽË?WöDÍò*?¿°¨«£?—™"iêQ?ï	Œñ•"?£ -U¥XR?iq¯‡Â?oþáÐʝE?œp˜}ì"1?¢,4ÄáN˜?íêDì»w?›žÏfïž?âèóÁÿ¤?~±ú#H4Ç?¬âöô'b4?™ÓCQ¼e?ìÄN¶ÇQä?¹Z)AAê?†ÙÌ|ªQ?míôª¹?·ï£Ï?CÁm?•ä?í›O]¥Š?¨³Èó8S?sܜƛ?—?kžRëÿ?±ç»F¯À6?§Ù6šIV†?í`¡I!˜<?¶"æV-0?€á#ƒ)K?Žž¯bÏE?²ÞÑGøëx?µ½ò0·íh?êûšÍ²?«ë*±[?'Ô]"B¸B?‹-óÍ$ˆ?Á¹Cÿše®?ªLÂt…î)?é=úi¢†?¥½ÖE­*?ã‡B֟?ƒâ=ô¥?È맖ºõ'?¥)ªØ¸ÉAGN4FGL J1731.6-2904?ïÐ謹@("[CóuÀ:Î.äðÀ;cä|캩@".çßCr?ÿ´o"͊b?ÇB]Þ¨w?£©Þ
aظ?à¹¡Kê?ûë¹Èä
¿ïø…'‹`?ïÍ/(·Ä¿Ä û¸•Ó¿¸Ôç"ŽuN¿æ)S¶`y½¿Ñ'ó—»HUNASNone?áþùÖ×N?ÅílgåÊþ?]\¹	"\?XÚîV"÷?ÝÀ¥S®u@?ÅëaÞþcÚ?âì¿u:-'?͇»£Ä?Œ-a¡«ló?—ç—ҏÇ?ÙE™ÆT?Ìߢ®QrË?áKµä0Ÿ8?³|r"f^?"žk¨?‹t
0U?Ü´!@}°?³ *&>?ä…
iC6?¨á³¯\ˆô?™$t®œ˜Ï?%iȥޒ?Õc£áϛè?¨D0cM–Ý?×µœ¬@Î?ÃÒù%Š	?i¾Õ^ú?a0Îø ¹?ärÔ!Đ?ÃÝÍ£êÞä?؟™½À?ʏaîmŒ?–G&Ûø-?£e"æ×1w?âþ7ÿ?Ê-êo±$?ÕOöÚ´¹R?³.·òìD?Ÿ^MÖ1+o?'Ñ`/j¦½?ä]#æ[Œ?³"©vA¶ë?Ú
5©ì3V?²¦²?B?¤üÂÅÎ0?"ZYÓõ¥?á«þºÁÄ?²`¼ÚƒMIXED4FGL J1731.6+0630¿É×5]§Gz@4®IäO QÀ:ç¦3ÛϟÀ<oyÌz@§5ÐòKa@)¹à<?×ê6jX‹?ïÿæՌŽï@zy5v'@Pԏä¹þ?ëŒÜ­¡¿Ã;—Æ/Ϧ¿ê
@?‹0J¿ïÿCwN7¿ïäÚ_²m%?ïâiamƒ;UNASNone?ìÛÒÁ®`¦?¹'±S»?®ªžeæv³?³´*»%Á—?£˜5€eì?¨0ˆ .û?ç܈•v…?Çq7Ê5‡?ÆÅH'#?ÃëÝý)iŽ?³'+6|£F?¯÷'j¥?éSk¡Cv?°wߢ†?¸ÊUOh?¥;à†â©?¼šR€o?î?§+€Qî?ç:£·L)?¯˜*'?ÊïTL?«žq.R?³'Â%™?›áÏ̋¨?ë"­²¼g?ÀçKÖ9ª?º¼â–Z?¼Ç‰ä<L"?ª{;b;:g?ªaq7^?ÛÞࠔ5?Ïå¹d²~?Ü­o†Âô©?ÐNž°?À‹c18îD?µB3l_R?ç	!©óÙ×?²¥…ò.?¿âBçå‹?ªDàOxž?ÃêX	<¥ß?«ØaaŒ'?ÓÀ:g?·†&%gl?ßЊÕd(§?¿Ëèîß?ÈÞ«ãYga?´ÖNÔÿMIXED4FGL J1732.0-2659?ï÷ØÉQº@¨5ÞßÀ9£Y#‡Ä…À:2K@]':ØC#@ì=áò?ÐàƒãÏÈ«?É=+Úy]º@ðAFm@­¸#®?áµ "µ7?ïøŒ8ˆÊ¿à0rÄBº¿å?þÞ÷¿ß'Øa*'P¿ðUNASNone2FGL J1731.9-2703c?Ô¦š¢ÇÚ?Ç^Ôký?–ƒ
V£Òb?­'ªŽÀj?åC"G}ː?Ǜ7¨°–?àˆ©•Ì@Ç?ÇDqt–?¨Ó-
º?¨ëìÁ"?ÛÔLNsf»?ŐÕ±ýW?Ú§žYòº?³eì¢Û?¸'챖?£œÏ³Jßf?ß4$¢^?²_ý ®¾?Ú¾íÀQ-3?¬ìwU)°±?¦Èªþ@Ä3?Š³–½=°?á3þo垳?­4ëÉV™?˖j&Ü°?À½ÛS‰{%?¤'õ‹ðª? ¶A–´s ?çÒD¶ÆÙ¡?Áœè:ˆßZ?Ðmy Â?ÂÚù¶9ãQ?·Taå‹?¸!V{?o?äèu¿õ£Ü?Ú+ì(Bû?Ð4Ã-^)x?®jê?à{ç?ÀXÐláÍ?¨tª$jé9?ãϖõ¿#0?±³•J'â	?ʑî¸\?¬`¯ž6ã÷?ªÇö£Zď?–à2Š_͘?篪~??®ê©€½5ÈMIXED4FGL J1732.7-2559?á¾4Ô¦"†@ÞµÛ¿êÀ9Àg{9\BÀ;?÷ˆb9±@ÿ‡ý@k§áZùK?˗©jÄD?ÔÂfa³Ï%@
˽Tn?ùÔ«JF¿ïÙ˜f"³?ïþáòο¿äjd!舿æð,µÿ+¿ì®a&ák¿ïþŽ`€sXUNASNone?Ë6nJ¥.'?»š è'àÅ?·ºgÊG?¯Ë·#\=?æP-ŽsB?ÁH§Ìë´!?·çºR»?À?-¶áAé?ÏU‰Oۛ®?Á>áŵßÔ?àˆÜ2"f?Á""^Zî?Ó8ÖJò9?°"ì"ÖÙ;?À§þiÛo?¦iŒ­N*?âC"•É€g?²ÂAJÑt!?Òó™+Ž?¢£'¼óø?ÊyK›^ëž? z"å@Ã?ßÏÁ#K^£?§+c¤øÄä?´$°æ»8?¦}á§Ï?¾%#8
Ö?µòõžó¸®?é¶É¾ƒŸ?»CM©ùZ—?¶èVm¯aÖ?±WݑG
ü?ÔrhÙàB?ÆK$¿Z¦ó?âéÁ1/šD?ÅÉf±%?Â*…_Ô?¥ÁÜ­
QÍ?Ķp?œè?²Ù1Æ2?æG۞PÑ?´óž^—"o?À®UÓÇø?œÇ0‰=^Ž?Ð
'`{|?¬F½jÄ?ãÍ¡[YíÝ?°-xF–EOTHER4FGL J1733.2-2915?暑…lL@@öÿÁßeÀ9(=5ëtÀ:}äÎv@ƒYdJWg@"šVWû?˱AÖäþ?Î^® º4Å@Xùã†M@èîüwŠP?éµâ¥|%ë¿ãu
¸A%¿æîZY‡¿æ@å£]h¿éßb"Ò¿ìu¦à©ùcUNASNone2FGL J1733.2-2913c?Ü4óòÖvÅ?ÃhégQÐ?ºœ£uvµÐ?´±›¦¶£ñ?Ý#ã/ËÛÇ?ÃMÉ9%™?ÕLéÂü¿Y?Ư÷ Ê?´hËâRVJ?®ž&ÈËô?âÌq¡ò[?Æ ƒ?×*è¦È_?³…lHb Z?º÷R¡&oš?¤ó"Ú?á¡WíÁ~?³ÎänÈîB?Âî"X«£î?›
SþïY¡?°Sj\ha?Žã%«\)?é:
UÅH? 6Aöl?ÍîÊk§ ž?»y> Œc?µ˜.*Lê?«Ú;<Ü?åãš_£dÛ?ÀBêwúÚÊ?¾ÐÖâ?¹*âbÓbR?¾ñÅ*
'?»Ô¹fyÂË?èGÁ§¡ü?EZI™ô?ɘCZj&1?«"àCè4?¿ñ¨¨šb?¥Æ™ÖÈÔ?固R6G?°ÃLåC¸¨?¥A@\Ô{Ê?‰õÙÅ(?´GQìÚ?šŒ'@t€?ì(CS'Ø?mEÅà^OTHER4FGL J1733.4+2235¿Ù–^?•0@:²ÙßÚƋÀ;k¬ºÞ¿À=G€ß֕@d@ÚÖb@ÚÂXÖ?Ӂ:þϾ?ïÿ4~ô€@Ù>½ªðÚ?ýCw£ûrR¿ãHƒýP"?ÄYbFò?ïùíÎ à¿çdU/¿ïÿۂr5¨?ïüQ¿æ4}UNASNone?Ú6¤¤1 ?ÊuçÃs1Ñ?àÜõ'‰ÃÊ?Ëgk²ÅS?°=Á[Éb1?®)•¿^>?Ò¥•Ø¼;§?̹[ëª?ãv4ùm%?Ïš'u?¹¸Ñ¥éM?¶RÎ-Dè°?ܲù\LÜý?· »=ċÕ?Ù@-Š°PH?·«.–#??IJ4+fò?©£M>Ñ?âÄ2ÉDÆÈ?º÷DÖ¯á?ÖÔÄúȹ?»¸[.WŠ?­«œ‰4³?—^ðút<ø?ќ·ƒ‡?NjÐV!ÓB?äñ™ç-‡^?Éî"ñäß=?² `#ªu?®NÓì‰}-?ÆVÇô2Û?É¢;…"ze?æ—ÎÇ_
ä?Ð*½²—[?¾"ùáFÆ'?¾ù6ça'[?Ô¬A¥*Ù?¹dö1œ›‡?ßæB
Zu[?¾:lëï/?ÆÚøÊ¿™?­²g´®Ã®?ÓóÂ",ƒI?¿Ž´ñ]¯?â-y*8bÈ?Ã6«5«ç?¾Å.%ŠÜ›?®Áª"loMIXED4FGL J1733.5-2950?î|mÌÄÎ?û»gšCÅÀ9–,­®À:í¡(TH@!;rò»Ê@âIC?ð±?ÊôþÑpË?¹6xð+Í?ô»k±)X@]¬Ùge¿ð?ïþ$É
$¬?ïö)óð¿äJN듿çÜÖÐ[͆¿Ã-ˆú:UUNASNone?ÚýOö¸Y?Ê5º´5@?'Ôҏ5eÞ? ©·¡{í
?â5ì
ãK?Ê`ÍË$?ßV–1&µï?ѾuòËd?Ó÷¦y­¿?˜brÚ˺"?ߜ*Tߢµ?Ñj	Ï?K?Þ§o«3Ÿë?´>è?²µNìLCû?¢Q•Ll?Ü«<™¹O?³VnîŒï?à»y}ÅR°?µØ«?"P4bí'è?‡ÅS[Ǧó?ÝD	½¡"B?µWÆúö?Õ@+_Ý¿?ÆÏ;`˜
?•79ϚâŽ?ªq\€âÓ?ä¶@›üu\?ÇL¥Wgñ?Ù¶ëZ½¢?Ï	7¥øfr?™DÄXž¢y?©éÜ°£)?âZÏgdpË?ΆCÜ"Ö?Ò­Y±ïs7?±Á©Yr
?½‡nHÝêV?ªýwѨÆ?âøe]ì‰?³²/5ÏO?Õr³ÝxÒ¶?ºœéÓ?™ób¥ÌÖ?˜íiò¯Vè?äw
üwî?ºç,ì¿}ÑMIXED4FGL J1733.6-2431¿æô=Te@hŽ^Òô.À9Õ]z.šGÀ;s‰½×g@0™@
ûÖ¥"£?Ëæá õ?á…X'@-+Ç.'?ýÑ}3'–¿ël{ž†é>?ïùÒSõJš¿ÛÆ~1ß ¿ç"ebZh+¿ì&îRz÷¿ïðx£ÌiUNASNone?¤+PÏq	?—'»µí?´£à«ûÅ?¬£ðý²ž?ì(ÎÝÀ‡g?°£®#Š
ë?Ñ·¼´´?º5å{U?ÙR"ÿï?ÚË]QŒ?Üä'¦˜?ÁÍR}?4¸?ÉãüY¾s?ªóoJ{ÿ?Ècˆ_#jØ?«×ŠXÎs?ãn\) µ­?²U"HÉQÖ?Ï®Û4ĂÑ? 0,C…î?Ñ´¢.=«?¡Ýð[+Ò?Þsð7`'?¨ÑF˜»"?"ƒF"ùr?…ÛÏnôœ£?»ÿÈ«3?²Cìᤧ?ì Uí¿®?³p|àhp?°‡
 ¶5?¯N"®?[?ÞÅ°Æ(e?ÈcÌQÁ'†?ÝÄwRŽ?Ç@ÖáÎ?»/NråáØ? a—¥œ³à?ÈÀðëºù'?±¡nTÓ^:?æiÙö´…a?³¶‡Õ»¢?¹»4ÁJ/?"1Ü추?Õùi…L'?±¬J¥"x9?â@³	?³!¶µ¾{AMIXED4FGL J1733.9-2220¿ÞeGÉSÃ@℁Ú`3À9Ÿ¬îàóËÀ;#J\D¤u@TÞ»·¦ @óà{Ö:?Ñ,à]Î<d?à€å7ýO@úuÚw°;?úÞÿI¡´›?ïÅÝÖ´¿ÜGm\¤Æž¿ê³Ãp=U¿íHzøÄ¢\¿ïÿþˆ0»Š?ïõÁ%y·UNASNone?ßä2ã	ؤ?ÊMòsœÒ+?Ð>¾ˆ!³??ŝE¾®¯‰?Ϻ'ƒ&¼?Ã[:¬?×1nb^?Ê«/§"w?͂÷ýÑÕ?Ä|Ô{«?Ú R®¬-ù?čí Ï:]?á?í‰ct?µª
yà?ÀJ·áO³?¨±®¯Ž?Õ¨$5X@M?³4aôGo?ÃЊÝ6
? ]("Ḇ?Ów0qšÖ?¨êŸšµY†?áPEwOå?ªy?%3?Òg½yÉp?Ĥ*…ÿLÁ?ہ7¤e?əÔZ"R
?ғÁÛN',?Åùž?¿ÈÑÛ?Á-•9•T?Ø]ôG}?ˋøQ
Â?ß°¯u¼?É\2êÒ¶
?Õ4IØ*æ?³^qŒužÝ?Çè	Uá€Z?±‹''£·ÿ?Þ×±}ø«?·;»öpë?Ÿ_P%9þÝ?"#I¿:_Ç?×Bt•>?µž'&ÂSÐ?ãcöDÈåj?µ.u"i¥MIXED4FGL J1734.0-2933?ïÿïI#Št?üø[ÆÐ3ŠÀ:Jøš°ðÎÀ;ÿGóÐG@ ;<hfç@2Ú˓?ÖöÕ^ìŸ{?ï?CwN7@
º ¢¢V×?ýþ0Çóõ¿ïÿø="ßE?ïÿîÝÃÀ	¿Ú~ߟã5¿Ö¯£#Ûý¿ëtcˎ߿ï´ì`»×‡UNASNone?½Ùl ð®‡?¼29–­4?Ñ¿—0ç1?Ì-'=å?ãeNÀ7?Î* +rä?«®¾"µ5?´ØÒ¼l(?Ý5'ÖSV?ʨp¦Jð?ßpԖ«å?É­ºƒ-?Úüþ˜ÌÀ
?²Gü˜eJ?̐gƒiMï?°4&Ä­?ֺͥ~˜ü?²›¥4å?Å[©ûLÎ ?¨?@Ÿ¼Ð)?åVÊ]lþÂ?´¶¿0ú@E?ÅI,Žÿ6×?¬W1fÀ®?¯`2Â5tJ?°œ;@?Øß]úª?ÏNÄÂù?ášN¨Yü?ÏOyƒZQ?—å²»˜`Î?¡ÑFIê?â8àï÷ý±?Ïbó+þ'õ?Úâôßîñ?ÎnPW\f?Ó]I«è?±+âMÓ͑?Òöþ!Œf?´á"Ò\
?Ú¤O*4²?´,"÷®ÊD?§™`Â@4?™ B+"âf?èüí-ŒÍ{?¹B"†+—?Æ%ó<¼õ?¶»¢ŽýãMIXED4FGL J1734.5-2818?ÜnSƒw/@[»èxûÀ9yÂ=ägÀ:ô˜"¶Ü@F3#îǞ@N¶Ú@¨?ÊöíÈ
˜?纽֏Ä@ð«†+(@úfÛ×+Ë?ïl-_ߎ›¿†ÏÊ¸Ëc¿Û«n®3"'¿í*__6p¿ÚŠ|›1[¿ïûr»UNASNone?´)>ê ›?²(s,@§o?¹Ë'SîÙV?¶I;"ß?êAm­¤àÂ?¿Úc–ÛØ?ÙçPB7³?Ï*·n?Àf,H¢?ºëýáåI?ÝåjŒ™'?Ê®'Deµ'?Ò&a/½)c?°6›ÒSÖ^?Æ'¾Þ«$9?¬IŸ&
•F?ábß°v¢@?²†W åc(?È1O³œz?¦Ôr¼î¯â?¼£ ß|/"?¡ÛKG	?æ_W#'ñ?¯eæ¬Ð`´?¨¬òõ}"?¢ìAŸ?¹Îõ}èZ"?¶zSh%æì?ë;R!=šô?ºèâEôš¶?Âáv@B:?ÄÕõ†e›v?Êý´‡l׀?ÄÞRÝXÇ?äˆ56Ô¹'?É/Y‡¹Oö?Åx蘟?©½×üÖªÇ?Åý³AõE?°ÅHÑg?å"Y	—¿‹?´W	Òú?¯Pv"J¿?˜WÂ7À?ÂvÑ`¸Û?²y~(÷[q?émD>He?´æ£~…þOTHER4FGL J1734.6-3548?ÞDX"6¿úýª…z'äÀ9Žœ÷+°À:זߪõâ@ /§zùª@bŸYÌúð?à•
ÞÖ9³?£N
ÿòê?ÙOGß=@ú±Â¸L?ï¼Ü)a"Z¿ìe€Y¿ä¡¿½ð÷¿ç8° œB@¿î½©CZÉ?à'F¿,%MUNASNone?Ì%v*Ãfá?Á10ÖrÏ?Žx"69j2?‹˜úæ¥5æ?è|À$È·>?Á·ºÊt`ƒ?ÛZZ<j1?Ì,WÄ.?ŠáI
RB?'"Cº­?áçL¬oÎß?˄o±Üü?ÛïlüÏì3?´6läßÝ?°Ñ'ƒ®a? <«ùj?ßÜ.b±•?³ÍK¢À´¼?á㐢hå?®õ~ßóµ?€WwË¿ŒÂ?nõgªB#?Ýq} <5?®Þ\ÿàd?»ÅÍKš)¯?´'c{~æ?‰í-*àG?†£ê?Yú?ì'¢2?µpƒxr?ÐVl?»¤?ÅXb?‡6"
rÈë?™µU¼éã†?ç›üAÑÓê?ÄùAӐ?Î0{2{R\?®oQ6Gr'?²ÕÓ70T?ŸqÎ×òx?æ&Ì6h·?°nŠoºñ?ÏѹZeb?°tSD¯
?€¡îã‡(E?ƒoÌ
æó?çÉ1ê.?°'²# MIXED4FGL J1734.6-2912?îŠ
ú-?þ2°ì©À9¯mO"¼À:À'\f2@!Jgö…`@`RP/?ÎË]k"?ª]TïÆw?åóø :G¥?ü‹Å~
¿ïW?íUÙP?î>3Æà¿ãí^½¥'v¿á*Vµï:¶¿àç'Áåèþ¿íõ¿4]ÖUNASNone?ÆÊMk˜ª[?»ºÍu-?QרèÕä?¢;EB­¹1?ê%Fœ­±?½<€¬ì:Y?Ӝ¸oG¶?Ëu WÆ1õ?œÝ܊G&?¢Ø SgÉ!?åM14'"L?Ë{º'ê¢î?Õqõ˜?sÖ?²"æb?Ó9?°õ/ãw¨? ³~r Ù¿?ã(_7ц#?³	ID‹'ý?Ó]}Ç߅À?¨'&Až"?•¤§bÜ£l?|Â>ØÈ£†?å¤áu?¨'âZ×ä?Át(#"5°?µËz…_Ùb?ŠíÁiF?¨ñ–¤ªkd?ë7>ó'Kì?¸à麱PÌ?ÈÇ#ô¦?ÂÆ7ípö?£*ú^é5?®BÞ1Z2T?èÆ^'/è¦?Ä"mR?Êe,ʹL<?¬®M¦i?°¨æº²ä†? ÜòLͳß?çQ—õžq?°zõÌÖ?ÀÜÀaüÁ©?£¥[¡yd?˜^†Iåå?‡"0ç
Æ?ëÛ´ú¦­?¤¨ž÷ÕΤOTHER4FGL J1735.2-1640¿ïDF^ç @ ú_"ÊÕ|À:*M)~~‹À;ÏžÙt{@4¶Ë®"¨@ÔbÞ©ª?Äü"_öŠ¶?À'KÊ-á?ùôàM/^@½Ï®Ôi?°4íóc?ï-*ÛuÝ¿ãj'ñ¶'!¿äM'àAô—¿íh!Äuæ?ЧÍęw‹UNASNone?å
@·DD?¿Ti—Pò"?—qã!kî7?0Ò%"H©?Ôn`_* Õ?¿"ž-°šñ?ê[e#ù·ð?½Ò&ÙÐ?"ÒhÆ|¡r?"|´ßÚÁc?ÃøXÊ`P?»º‹ÂŽ³?ê)^ëó®Ž?¨ó`ªÁf?£¸Û œ?"#Íp¨â÷?ÂlMh
!ä?¥ôp±—1ø?ëÊKE×-?"ã—"Áp?œ'W
g‡Û?yÔKï\6¿?¼w×äK?'Wˆ#»Ì?Ø؈ùt†Ì?ÁëseI?®J@N `?¤§ÙÀ~Ÿh?á¯ÿN™?Âí4v?äUt_½¿?ʌ,‰ùÅ?¤g˜Y} ?¨b£Ã?ÔÈ%Ž.?Ʉ]\Òhî?ã†ü
ÒìÌ?´.¹w– §?³ŠAÎ0Ä?Ÿ•}_"@?Ô+åZ§U?²˜ÍZ« ?åÅm^
˜?¨,ºTAy1?®Ē®¨P?'|SÕÀ?в±X?¦(Dwì/EMIXED4FGL J1735.3-0717?Â'¢xåÅ@*":귙_À9iݞ¬(À;l`Nq@2pÃa"@	ÿ&ò³?Á0/GÁ4¾?Ð0&£Ø·½@»)'<†@¼ƒ †]R?ïÞM}·:ê¿ßøQ{¿ä¥žŠš"V¿é+î›S­ý¿ãœ/vQ¿ïö¢¾ÜIBUNASNone?ê±Xª2m?µÅ1L'»?«2ÓÍ·?¢2«;<?¼ò¡ª•¹?±¹d_,½?äò–F?ÊQwÝú?ˁ€¼0¥î?ÄÑî¿æµV?Ä´ëbAÇ?¾†çEsý?åî×5 :?°gG§w7?¶'™£]U?¢Li/?ÍHÊ.?«rÁPñ?Ûp<ÂÂÍ?£2Úi_Ãt?ˀL–†"¯?¢Î—·s?×"iwùòÜ?¤*Ò^ˆ×?âUZ!DÚ?ÂHð"¬8?ÁQ—"h?±³Ø~?Ò­Çèa~?Á®—ò?ՋÍä$g?Ío…ōyŒ?Û¬Sy¾v¸?΋,A;Æ?͏½D;Ã?ÄUÎÉQB=?ßÚV£$Þ?³~8<¢ì«?Àµ@ýSÛÓ?§Áô"'|ž?؊…*²í9?²VÏÞcÈÞ?ÁåumÈãè?™áàzì"Å?ÖµuëóY?³%ÖIwô?à+箔AZ?±š›Ý奖MIXED4FGL J1736.1-3422¿è¼wÑ·‡¿ò¦J'ÛÀ8ϙ O–@À:ùÞØh'@üpí(@ÐÔ¦2.?¾ÝþMxX×?ߙrb+Š@:Zà÷&=?ÿ=«‰Ü[?ç¹`>.8ø¿áþÐW›È¿Ð•ŽÝ}ôø¿ââ7ùk'¿îõ"€-¿ïø¾nèìUNASNone?ŠáÂ֓oë?'†Ñg|–?ê]^®H?½Þ̔π?ÄÜiEÁÖ?¼*n
%Ô?›Œá³
o?¤6åŽì?àt¶ßb?Ŏµ÷"D?Ýf‰s©~?ÅÛÿ´o?¨ÝÉLÏ?›µ
a£v!?çW-ÎÅJw?²ÝJ¯ŒÜ-?̟Ì.¨p?°ç ó? ïúVüC»?|'è'×?Ö 7ôÊ(?«¸£П'?ã ä`+'»?¬ve6:¥?…M¦`ƒL?†<öîmã1?ëhº¶l/ ?¾‰oÚZm?Á`J1kL?½
aº§}ª?…$®÷Sýç?ŒêږôT¤?ßøLjÅN\?ÊvÇÛT½?ß^Žî4?Ê*ç:Èd?˜Þ";UÄí?¥».øb"?è±jJ‡v?´>\5Ú½?ʆPÅ	?³pšýè?'´âÂ?e.ì	ç?؄LÖGtß?¶¤rÄ ^x?ãs–n¹>?¶¹Ä;LÀMIXED4FGL J1736.3-2929?îY(2N0å?ö¹ïô8À9'7›wÀ+À:¢êºô]5@ç+¶'"Ø@FºÜà@G?ÎUíQy?׺¾A@
†ðÝMM'@1•@C'¿ïÿíUÙPi?ïÿ¾ÇPŒ
¿äXeAxEa¿æړ)=,¿î{J#9Àì¿ïÿèþ†®/UNASNone?Á†Am]¦y?½¤ÈÄ ù?Îíªa¾ö?ÄçXÁYžy?ããH&¤?È®H¹})?¸£€55?¼0vTðó?Åç`	]ª^?Á(Å	ù—Ë?烳Øè†?Äè®®îYS?Æh¤_¬t#?ª<žþì?ÍÏe-u&?±P–ÚX?âñý¡‰…®?²oâÖ=Ô?ºµIð±Oæ?"t¯}t?Å@k.f·?¢Ë·Õé?çY;öPSÕ?¤ùöëH&Ï?ºy"rkµä?·$šÔ'"Ú?Ï¡'í¶?ÆЀ¶sÄô?äȃÐ7C?É;Pa¦?¨%u%3$Ì?­ŸJý•?ÐðSŸ?Ê\dÒ4C?榃É	?ÊÜJ{ÊÔ?¹¡–,¡l? k"ËeË_?Ҕ׉ò»?·÷§]½Ðz?まN¸Ru?·­x¢ф? ;§ÅÞq?"×Q¦‰î¶?ɊjÎ›j?¬«ÿ1Tß÷?虪ßÎB?­	@[êÖ[OTHER4FGL J1737.1-2901?æa×ÈJ8?ø†jGœvÄÀ9Ž™‹VáÀ:b4¡È<D@«šêÒqQ@!dԕï?Ё^ú·@É?ÓÛÊ@«kÔ@¯d9Ö@
7_½ªÆ?ìó0®ôt²¿èmÝ¿è̞
²¿âZ£"Ôæw¿ï鲀ñ,(¿çKù"k9àUNASNone?ÙWɯOÓ?ЏÆ`2?¶¿°NyÑ ?´±·à#
C?à›Þ²?Òxþr-¼?ʎŸÕ?Ân‰\úF?·ù)–	=Ø?°€n…ë?æ]Tå"à?Í݅¤¸?Ñ͎ä3ñŸ?±½"<P
?ÄB¼¤œ¾?ª»‹Uåãë?â¸^¼à?³6'¿í©,?¹D>#ãEE?•»p*ïÊ?²œüRòõ?"´jöÖÒ?êƒØ±KUÙ? µ$??Õ[0uÇ5?ÏÒ@MM?¼7e«c?¹Z{Ž¦'p?á˄8gK?Ó:7'Ø?³Ù?¸+ôÞ?´y€Q%C?¾èb"G?¼"ÚFv˨?é§×üÅ|»?Á{Ï2œy7?Æwþ$™Î"?¨X
AÈ-?ÅôŽ¦ú?­#Ò©@ç¸?ääýS0a?²š…Ä"úÄ?›Ô¶LÄ?'¹'oUÜT?µà/™wj-? SÉYãl?ìeTZA·R?¡Iõx"ÏrOTHER4FGL J1737.2-2808?¦²Dó–?ÿÉåA7Ø´À96"S.{>À:Ž"%¼R@сd®M@ßdš?ÏËø&êþ?ÁB%©Ý´|?øXà66ò@²°ÈŠGí?ç
«NÍÃm?Ú#‰<TD%¿ì¼W3Ã{ë¿â¥¥@–É¿çÞÉ^®64¿ïÿø="ßEUNASNone?Ü\ˆ¹nîm?ÆôŠÝOb$?¡¯Ú¦?ž¤Á½e€×?àÀ ¥ì'?Ç'[½Ú°T?ߧ™.E?ÆÿdËAîs?«vB=Çs¸?«då\æŠä?Ü鞉îUß?ÅnJWß\i?ÛÊA‰¯Ž?´Ï‰N·Œã?±Ùcz	»?Ÿì›dÃü?ß¿e˜Wœ–?´&(m8f?Ó̧Ì?çª?¦¥jÚª¶?¦ì±/í–a?…'§"T=?äªá·÷u?§*–ñ7?ÏS%}y9?Àë ¼<u–?­áŠŠb8?ª¤2›Pˆ?æM#LôÐ?¬سl?Îó+±3¿?ÃEfbE֊?»Ë|.¶?¼VYÓÛߺ?äâû°ÃŠa?ÅO'g=?ѵ–9è¯?°SfJrü?·8õ{'ú¬?¢Ê?·w'a?ä>3¦©*?²\5!F?¾Ä©¬{€?Ÿ¿n"D
ü?­ù%:_1?"ëºÓÄñ^?êGØzf3Í?¢f9Yz»MIXED4FGL J1737.2-2421¿ï¨pŒ°@
F:À9Ê/¿á+ÿÀ;|ùOâ–@ |}Šsï@èËùh6J?ÀËCòž¿¢Üü@q¤?æüC͇Þ@®r/QŠ?ïË:%•»¿¿ã¾>ê¡t¿ésòí†+¿çqÿÅG¿èVþ"p?Ôåè&Åf§UNASNone?Ö70ÔðC?ÇA`gc?€€V†ÝDã?xŠÀÇ0¯¹?ä¢f;•¤º?ÇHøÞ3ã˜?â†Sgl\?ǖ*h"B?š®¶¢™?œ•ñ@
f?ÙRŽE†$¥?ÆÚ»~W/?âñí"[?³ùýckÕÔ? ùI½Å:5?"…–HÜ?Ù®ôŒPÓ$?³TužQ8?ß—[%ëw?¬rڀÿÓ?Œ²ƒL/–?q/'ˆ(é?àé‡ÿ¤w?¬{L-~^?Í^6üa¨?À.I(þ?Œx'§ør'?ƒ€t´þ¾þ?è66ˆA?ÀŠÊ|ª9?ӋX
]5»?Åy ™8ÜÒ?¢
Œ<b&©?«×D®‰?å«5´~?ÅÞ-‰óUÅ?ԌÌ0 &?±ö6YО?¥ì5QSVU?"¹
"BË?äZ֒ô8÷?².J?ÈpõHõoâ?©wÀ1+ƒ?•¿Ns¦K÷?†àEYä={?é5È9ü6X?ªqKnSÊÌMIXED4FGL J1737.3-5300?æNQû±wîÀ&`'ÏR¹
À:–n6>€nÀ<)RáP@Š¿â@inù²Þå?íÐȯܧ¿‹‡¨3
ñ?É–¾ÈÓ@œÄq^'?ä «†+(¿Ú§a£‰¤¿ä€ƒSld¿ã#ý5Je¿æ"!Í°!›¿ØûsT‹sUNASNone?íž—"z?³Búïëwí?i­y2¹k<?bÛ­>u?¶M£C]ð?³ª.¶M?íS[îNé?³AÝ°Þå?c3÷Œ¿š£?i²€ìÀ?´Ë€Òþ^"?²ç…Tx?îC`¥1R]?"ñªÓè`?uä{Qw?eÒ=C'?©
f@·çI?"ü±–'?î½|ñ©aI?uµ5¶V!ú?iqÒ6¸?H`]=hÛR?¢ðʁ?u3UN²[Û?ê˜
-mª?º€†~dñ?|˜Çš²k?pWÓ_eÑ£?Ä»ŒÞÔ?º–/ôr?ê'Ä+?¶¾[gQ?lÙèÉ;B?|Zɝ
Í?ÅA‡ó¥ê?‰e†ŽòC?êç€\—í?¬[ûí5rà?‹Ú½:'G?{ñ֊Nl±?¦*:?«vnÔñu?ìG¬+cþO?'ßµc¢ÝR?×â]Ì?i—héÚÃë?»‡»`=ØS?'žå EìAGN4FGL J1737.3-3332¿ïãÁl,µ¿íã¨TáÚÀ8àòFÀ:vIë	Ï@¯'º@K•"d~?Åúq¶%Á[?Ú7ÖÛïTŒ@—›ý÷è@¨0‰à"ÿ?îØn¡Hdž¿Ù¾(Õ!°¿á¨ª®"Ó¿ës³‹³'	¿éFõŸ<q¿ïô™=SHUNASNone
?®0ô¢PbÉ?«šb²ËÆr?¹&n%ÐÞ¥?½ã‡íR[ö?êø"ñ?¼Q_C1ƒ?ÁN"Zm?»wj´mŸ/?¶ïs&#'f?­.
¿½7?èÎl"¸‹ø?»x—M[tè?ÀRôn§R•?¦LɟUL6?¿@ñÄJj?¥¨;~vº?èB†¢?®b¥¿?«ÛÍ(Ü%?ˆdԗ¦¸,?¿*ST¢ç?–'œ{õd‰?ê](«<Q?›¸¼wÿÐ?žs­D)!? ¯"­¡Ž?µ«³¬e/L?µN=Erà?ìVð½÷=?º–C-?¥ˆ±;$	?¥L÷E"?¸aч­Å?³#¼¼Zû?ë›:»_3?´ˆ(‡p"?´wW‹%dH?›†º9RJ?¼À'á>t?¤#ùÀî?éÙ\Qm9?¨ßé'×íã?‹X'"'Äm?qܧ¤^ð'?Ã/Ó;j©?¤»4wj–?êÆ©'Iý?¤—|…wþ³OTHER4FGL J1737.6-2350¿ï	^½>~@ÃNü½UaÀ9³ç't1*À;S~3Æ@m]–^%Ð@N€F}?ƾ—jjW?ÐÉD'@	ž³íQ@Ku&r°w¿æÞKòK?ïäÍ_ê2¿æ;À½Iø¿ä­Çüƒt¿ê2QáÊ	ú¿è
GŸUNASNone?ãmf«Û'?À¶u£×F_?¨ûÛ-Ó¯? W̖WV?ÖsÏ'‰?ÀÑfö•Y?à{f>è?ÃË	h´tf?¶¼Á-Z¡Ï?±Ãæ¶b:"?ÙZ6kKþ?Á:¤IS?äL¥­y|?±%Ž,£?°Ñ]ÞHt?šF¿iT0?Ó2]-`>?¯ø•˜!,G?âêj[àÈÐ?¤CûÖ?´K<ÿLÂJ?Œ5áÉÄ?Õ\OÀï?¢S—$?Ë"+P2>ä?¸ýPÐI{k?¾¦NÚiԖ?³GȪ¶ôà?åb«Q/¦?Às–•-N?ÑQ¶o×î?Âö-‡¢¡?ÄÌ;ïç¦d?Àe¹5=?â$Ìf?Å ¡"Á›õ?ÓT;ÿµ'?²û£jú~?¿˜ýðä·®?¦tÛ¢'6…?âbŸ¤lþ¨?´F:÷ͬq?ÔA/¤w1ÿ?¦ê+pZÖÇ?ÁŽ¼Èë
L?Ÿö¤÷¬­?á{¸ü
?ª¡µd.MIXED4FGL J1738.1-2453¿êÅu™Îâk@U.€F}À9&ÏEM+À;"£Ð_@)Ö=8ñ@.v»H@?Äx"%çEI?昚ËÈÀÏ@4‰¾ZCB@(ç-÷	?ïñýwŠ%?㲟YÌúð¿äpYߚYÞ¿ìÊXÿ°J¿ìb2Yï_Ÿ¿ê"tÔ¾2ÖUNASNone?±â0:13'?²Î E+?æäÁ Nݑ?Ç:ºæñ;?Ë{ãatö2?Ã9òÑ)?¯g.÷Q?¶
HkhS²?ä~'DØÄt?Æn¾ÑÊQ?Óúóўn?ðëž^?ÍÃÃ+ìËx?®"Õ¼2ìT?ؙsÙìp?³´¤ì?؄ª*D?³|<fÒ?§EPJ¨í5?"c
Üêâ?ådxRL("?«ùP.-ÊE?ÒNeR.ö?©0¨ÄxÎ?œ¹YÕÔ?–ày@Íio?çÂ/üá¬G?Ãâ}Ôþ/×?Íu(áu¦J?Ã!" ¶"?›Qý.܏Í?ªS3??åhãÙ®²…?Ë-3þ"?Óyyb[Y?É]ƒ=⎫?¼"gëC'?¤qqkú?Û»;)÷ 5?¸€Í¥!ӈ?ÝÃ|
?·ð‹Ýö8?ÒÚJ"D?jGವ×?è7ȏF?±ï€H~ë?Î –oåã?±wl<ZMIXED4FGL J1738.8-3241¿à)֘}Î¿ç–Äg£}HÀ8ð"¿?EÀ:'o¶q@µ@uU«ÿ"@ZÊA¤æ?Ƒ®éŒöô?Õí3	AÈ!@	]®f°8B?ï‡îÁ"4€¿ïŊîÛëN?ïùvÿ:Þ"¿×¸o}f],¿ébü¹úb1¿ì¿Í_ï©Ç¿Çè5žrqbUNASNone?»Šª"fú‹?ÀZjŽòª?Âj²Š"Ñ?ÀûDº@ï?çô
Àð—ú?ƌ¯Œ?·Y≰?³œgö8Ÿç?ÊFJûY…¶?ºaÞRu?æƒ1Ÿ?»å?ñmÒ'?À‡õ­@À?¦€Ìë–ìŠ?'nbÓ"?¬¤Ç
.âx?æ–MÐK?±¦bÚߘ?¦£Tpï?Špv5§²?Ǐp~$À?¥öc+Î%?è±î•}ñ?©Æ<âIæÈ?ª‡!Œà?¯+ŽÉèß?½ó;Fî¸?¹á
e]Ê?êŸÀ+B'»?¾Ø¸ŠÂބ?ßÞÒ|ÇÎ? ØÿŸ®?Éû$þ+|?ÁcÊ~,3?è'7Ê
"r?ÁܟŸî?´ÎRÍùÝ?R‡ç^<?ĖÔËÒY‡?®9€j£¬?è@€‰Zå²?°Ëþà&?Æ.{}Æ?vÄ°1­?r?Ê¥C•oØ?³!5W‰?èߖ`¿?³²GFð½2OTHER4FGL J1739.1-1059¿Þe¦'¾r±@%7â–é¼À9êuWšñˆÀ;r0˜N?ÿ@s¸7ê@P¸d_ûé?ØÐ\Ä|Y?á¸é‹It¾@7褙§Ü?ý¾îUÄE?ïþèÞ{Jú¿åöŸcÝõê¿â^þ]hã¿éùøuȿ뵃Úët¿äHŒ`ÌUNASNone?ä¾zà?Âû-ùŸ?¡/Ø4ð?š@BT'8m?ÔP;÷Òßá?Â|®q—òÐ?âç)Ò·G?Î]µè¯¬V?É0·ì.×?ÅpwïOc?Ë3Aûñ¯?ĂØØãÁ?áQЋâæƒ?±Ò«Œ7?¼!T…ࡍ?¤n`{'è?ÖT	ů)×?°»¬‹Îk?ÎÄRæèèó?¡¿íÓC
»?Ï ålš¡Æ?¦[V/:ó?à†±ëR?¨¶Të]¿J?Õ¶A¤©ÜÍ?Á™‹v$?µ‰7£ÕÇ?®…wþ³1˜?âs¸L?Ò1?ÃP¾ò¢'?Ò+KՍÝñ?ͺùl#O÷?Ú³ÃzØR+?ÐZ¤Cõ+?Ó ð¯™Ïä?É7Áj÷xP?Ù–×a??±þ|°^?Ã\8/q\º?ª_ïRÝ5?ÜÒßP]¦?±:ê5?±&
ã€9ï?'³¢˜ì?Ññœ¡+?¸î­;DÌ#?åVÅÕ?j­?¸–‰*‰âMIXED4FGL J1739.2-2717?éPx`;K@n½ÚÁ'À9UçòÛÀ:¿Véá@Y×p"½'@¶Iû̔™?ɟSÂÊÀX?×%àº?@Õ"~°	?öãXAµ'?ïGˆÒy¿å¥ƒb¯É¿á¡—)|Ñ¿è[@*<•¿é\žÊù¿ïÿÕ"[ʁUNASNone2FGL J1739.6-2726?·û[øX©«?²†Í‡ÇYý?Ã!ϊ'?¸+мk÷?è8LÍ¢s?Àä´
ýÞV?šXì¼?Á_ÿ+Lh?ÄÇy"Xó??¾((÷d?æ' —Üø`?ìõC/÷â?Ëͼ_8?¯Óè4‡F0?ÂSÿ¾^ƒ?¨N8‹üg?äw»aP¹?³!·Ï~:?¨ðLŽ›?"dĺ‰p?ÆÂßùzTÛ?ž·7á¯<?èÀC8Ü6ï? ƒžÐM%q?ª2…(ã?¡ô÷Àï³|?»»7	gÃð?³;Ëóˆù8?êåw&ŽEd?·'¤øïÖÂ?§ø?°^Unô	?Æ3†L,JÙ?Á¥ãÁ}ZÁ?èó|4Xø?–(¯æPñ?¾-À—N*?£s$.ÆWŒ?Àˆªq`Èö?¨DlS€Ô¨?è3ë"ãý?°GBþî?‡Þ=É X·?n}ÛçµØ?ɸ,õl1?¦»žñÛ²?é2|`ÛÁ?¦×õì'õOTHER4FGL J1739.3-2531¿á÷'ë#ÇR@ÖûÅÜmÀ9ÚÖzËxÀ:ÉŇ^.@`æzGð@R):‹í	?ÀÄq‰…$m?ֈ$;ɄÄ@©(¿;ê'@‡rÑÙ¦û?ï÷º· "¿Þ}nàÞQ¯¿ã ³iNx3¿æ:½ …«¿íÍӒ¹«ˆ¿å¾Anµ?UNASNone?¥¢NX"yÂ?™:ò¡
æ?âN1=Ã8?ÅK'ó˜q.?دÒ<ð™?ÄÖKþ¨‰n?̪JŸi?À=ÂÀ7?Ñ8ᇴ?¿uN©¹ÕØ?àwùbpÒ??ÂY™ð,?ș6£¼Cy?ªÙû?™ ?ҁk#~N(?±'ŒˆL°?à˜üÅQÈ?²Ò5 Ü	$?»ãÒÈ>?"‹·å§<¯?Äù)§]?—¢Fñ"ò	?ç_¼»T á? º6•dìï?£6ãù?'Ð@P¦VY?áæfÙCm?Äz»Ä"?ÙÌWdžmÇ?ãâ"W?²‰Ì•®ù3?³‰ïš#¤—?Ô{ zÒaÀ?Ç!ê§dn¦?ãq60
+I?ÇÒÞ
Y?¶@ùÌQ€?Ÿo_Y7ñâ?Öõ3×%žÔ?¸¶ŠÃ¢]Œ?á½b5)†?·Ée0¨¶º?[/P¥‰è?€ÍP"ˆä?ÉëŸQOº?¦¤fÆu?èš>±&å-?¨%ï¨ÄÚ»MIXED4FGL J1739.5-2929?è²À=¦	?ëÌ¢q¯À9{'±HÀ;MøԒ"ì@5#ä`½/@$Þ˜¯?Ғ(ÁÀ)P?ïûB+ºü@úô­¼fM@«À›<8¿ïÿù³>†?ïÿ~'Ø	?´ÊÅ㤀¿ì51ÛD^Õ¿é8›‡°c
¿ïÿ+#š8üUNASNone	?¶Õ«å€à¬?¹ìO/N]l?àsË´ýUß?Îæ–Ë;°¹?Ùbýœõ?ÍS¢"˜õô?ŸØ0b†M†?«d¥¾bs?ÜõjOÔÿv?È@øÅÆjª?à†‰T…›é?njZOñsº?̱S6UHÿ?­T®1oþY?Ñ´°,>]š?±wbõqo?ßò¦8–ýæ?²K€±9Ñ?ª
á%êô?ŽL%›»Ÿã?æž&ꃷ?²,øs©!?ϬÎ÷¨?° xT"E·?¡m¬dy0«?¬ÅP©NØ?ߥ;Nñ»Ö?Ï:îmÜQ?Þ-$,§u?Ï$ )ÚÞ¢?'Y&¼÷$Œ?üˆˆA…ñ?á?æȪ?ÎE‰¦KG–?Üj ¥‡ö?ÍÓyusì?ÁF£˜ÞÖ?§'ÕOß-¦?Ô Ø¡±?¶_Ôw4@¯?á]êÏAFF?·K?‡wQc?vBÜm?è²1®¬Xí?µX‡e½?Ë¿ÈULkF?´Ï®câéMIXED4FGL J1739.7-2836?»Eõÿ1_/?ôW½;_QŸÀ9Ë
F9 À;ºB¿˜0ä@ W·¡íP@i¾N"È?Òë=%Op?ïü ¨Â@(¸®1×?ý%@œ'hz¿ï÷&b?eF?ïölmçd(¿×Xï»^h¿Ø•o¾Sã,¿ïâa9Ö»?âN¦±\UNASNone	?´Íͅ‡Ón?«àÕ­?Ô‡>à2?Åpœ?':z?ã]Ë™?ƶâL2U	? ‰Ëâq?¬@t³\î€?â9â©Ün?Ë"ƒåŸ£ì?ى©Œ€×V?Ê1é9ȁ?Íy•=ûtf?­!ڀ –'?ÓÐ8Ž"?²üÝ'3?Ýs2Sܘi?²æS42?²µ¸—JYÌ?™·1T`Õ?è¹Crñd1?±½>Í5Ì?ÃÀé:/–?«ŽáMÆ?¦½¯(>?Ÿ}VÚ瞉?ؙ#Œú?ÈhE·wى?âG"GÎ~[?ȍXpIŒ?Œ>
Q½Œé?˜ÜŠ?œ?å'Ïæ\ÀË?Ìê-#jl?Óøoà/!£?ÌKàÇ38o?Ãrè'	¹M?¦¶žlz?×Wkƒ©Ï?¶›ÂH!r?Þï 2¿3Ì?¶‹Áþ]U«?Šj'{Äí?€%Íû''{?ëƒk_I'™?²|'2›Gj?ÀK°è÷?±pF'™KêMIXED4FGL J1740.1-1928?Û-'«äu@Œ¢:RÀ9E,Ñb¨À;ÀJÞJ¤@×ï½èƒb@#é Àiè?Ê©œ)&??ϲ?WÙ±@§~"ƒÖ@Árážëé?ïD8>4ï¿ãu]ÐÖ¿êøÛH"¿åŒ){D¿ïÿ>¤€}i¿ˆ5ø=œòUNASNone?åö,žˆZœ?Ä>`£Xà?´¤*¼‹õ?µ®Dç½v?ÍÕ8)ÝT?Á˜Küh?ßWÐêqV?ĽÈ(‰r@?¿ºi2sš¬?³ÔÕW¾`?ع"ÈñÃI?Âfgå?ál¶i*ˆa?´Xªž?¼¹cl­?¦{–ý̹?Ö!¤ÔÏêR?²Nx}¤¢?ÝíNÛbðC?¤OU.®ß¿?Á>õé.?•\pe»2?Ùsª¢&?¢»@Qä*?ß:Ó8Uÿ?"úU=–†?Äà×ñ™
?¼aœZý°?Öº¼[‡Ý|?Âùôņ©Ê?ɧ~»0B?Àš¯¢?Í·lü‹4?"ÈG4¥'?â(E¦ï?Åt9^¦Å?Öt€‰Áùú?±uÛ?ò°P<d?¬1ëä®Ú?ß²'N<gÔ?´<SiõÂ?ÆötÀ5(›? >"±¨?̬bKFæ?¨þ%ºm²?ãJ=!.à?©TS¥½MIXED4FGL J1740.4-2850?ÌËÊ
ƒD?ð
Ð"¢§À9†ñ·û"À:s¯þ_ìÐ@"ù‰@? §??Չüm¤HI?ØÈáè@
'h	ԕ@{……e…¿ïÿ2Döª?ïùÍKw͗¿ÚCC ¼
7¿â˜ÜP'`¿èÔ6¸ù±1¿ïûgêÊä•UNASNone?°ñ7r—~
?²àúËö~›?¡ÝÍÿf?¥u'?ìÑ¡Ð0H?¸õ¬a±?È\'j:?œ‡bE«—?ªA"¤K?°^ò˜})?èU©ƒ¢P?ÆÜàýA›?Ó TùÎÛ?±iŒñ}w?Å®]<t0?­AŒpÉé.?áa…ùK'?²ÓÕO÷:ê?ÈJ©uÉt—?«{(~" ?•†o!?z¤/¡º™©?éE)rj*Á?¬ëø 	K?«Œþ`ۜz?¯†
Œõ'?ÍÓ3ÎvŒ? œÅ½ÌÅ9?íXÁ€F?´j¾A/$z?ÀŸÚ7ˆ?¾iç1Ip"?´á†,gW¡?¼ÉØjKV?é<	îȺ?Ä)
<'M<?Ì."–ò?®ÏSôJŸs?Å1·Š<Ѻ?®AG¦gˆ?ã¨	w´'Ì?´T"(ӏ³?´·7¾w
l?¡×+S'ê?'Ýd
Špö?ƒ_ªÞ±ì?ìÒ-çÄÊË?¤/ÈP®q­OTHER4FGL J1740.6-3430¿îy3òàÀ5ĊÞìÀ9ùóEÀ:Í£ùZÊ@‰éOdl;@‰â¢!'˜?ÅÐ2²Ú³??Éédµy@ÿEÅÜï?ÿEù ½º¶?­ÇN¿èpöa7¿çBYì°¿äö¦_¥¬ø¿êõñ‰D·À¿ãĸ;SéUNASNone?¿EÅ}p?°g ¹à–@?«:êâŒ|¦?¡dÊHÒÆ{?êc°ð^ˆˆ?´Àæt«˜?ÕpÉä?ĺ\6%š³?¨â6Gc?¡ö6·þÝ·?ãû¹wŽ	¡?ÃÝu|Ä?Ó[ê^¼#?²e©®ãÎ?¹&®KŸ"?£*¨˜a¡‹?ã-5+A2‹?³'3`Àå?Äë
•øÛ?š>*ªæ&?´á¹Lã¨?«#'?è)p¾jE?ŸCÀw"…:?´U,Ù`í?§v¤õ]Þ¯?­¦@!â?¢öǝèý"?ëšò]˄?±Ù.Þð?¹Ñˆ¯w¸"?³ÙuÜú·?®/W[†Žz?¬»g,Ö?êâÙtX ?¸aTÿ?ÄBËdW?§u´_.?º˜K6›XÈ?£J&»fÚ?çœCӍÑ?­½"‰è'¨?¨×N?‰Ç1À2Þ?¸ù÷P6¬Ã?—ø#\ß?ëSH;Ö#?›œ/ÆÎ"fOTHER4FGL J1740.7-6750?²|>NÀ2¯Ë':)ÇÀ:ƒž…'À<&c{Ð[@ÑA}£ÄÁ@°ÚB×%?ÂVûºKü?Ï¡Îò@úœ@"0{ÈÎ;@Všó
ú?ïý«&‰×…¿äØڌ¨ðO¿ì{¯¾Ÿ ¿åЭÍ-DÝ¿îDý[5¿ïÿߞ¶ŽóUNASNone3FGL J1740.8-6755?îžy2??ŸSe:"æ?#~"˜no?íÖі2?œ
[(é°?•æ$ò¼C?첺¬±â?¶çwA+Σ?®‡<ún?±Ì+_­¤?¦½Î'üÚm?£)žÜdõl?ëxJà+¬à?¦¾âË´h?®‡¯õ;-?žÉ‹nB/?´ùÑ_­o?Ÿ‡¢KCö$?ëȂÓYƒÕ?"4í°b¬õ?³½¿¿xDm?D	!ðH[?«üSG+¶Þ?ÑUšÖ£m?ìÑÒx¼?µNîlpä?¬ýLR†8(?«¸žŸ@a??±lÓI?¨òOªl?ç¹÷U ?Åîƒ8Q?ÃÔì/WuL?ÁÈéÜZ¼î?º†lý?—?³¹¾e†Æ?èN
5 ÿ?°(æ\£–‰?¼
ÒC·ÃY?¨ÜzGwkz?ÀÀâ­MšV?¥VŸÈ'ŽŸ?ä"
Â.k×?«Žl{¥F?ÌÅà6-…í?«¬ÉlÞ	<?ÀíôÁʸ?šc'5AGN4FGL J1740.7-2640?Ë:Ý
Y&Y@ÕinX£/À9¨‰ò\©NÀ;L'݃Ô@ð¿Îâ{¶@;½Ep?Ñú"å$²g?å7]ú14@‰0«½?þûþ0Gœ?ï«íßl¿⎧Þ*î¿Ø ­ŸŠõ<¿æŠw½¦¿¿ïÑdBSb¿ïäó¿ÕÃkUNASNone3FGL J1740.5-2642?¹ƒ÷\G†?¬i›ÎGä*?ЛLgÒÇ?ÀÄǾ‰Ø?äÚáŸÌ?ÂF'+½óì?¼¯ùËf"ý?Á±˜»?î?Õ%Œe?Ä.Þ>Y?áÚ{4un?ŕ%©æK'?Ãß³¦­v?¦ÿ@õõ'?Óð¤
"a)?³gƒ
Э?áC¶
Ì$?³ê_')zþ?³©ú³yo?Šƒ¦‡ —»?Óºkź£™?©/ؕðÒ?㭊ÆSG6?©ã ‰á‹?¥ƒ"¨{?«\Ižùc?Ëu{¤ˆ'g?¾þ@³à}ë?çÊi%¡_?ÀÜþç.Ö`?¡Â‡Þâø(?±+"Â7?ÔpVûËy!?É$f
dÌ¢?䫬—
?ÉJù^·Vª?µÜüWÅ]?›:ñXø]­?Ò«ÿA¡?·ñgÍùÛi?ääÀ*õD?¸*ÁEÙHÉ?—ËËÎ}¯Œ?yVýó¢Wæ?ÒÀ"ÛÞHÜ?²È6á6½â?åá3œî?²À¬ö‰,çOTHER4FGL J1740.8-1832¿ÛôW;ŒYP@kÓ^·E|À9ÌY…­S‹À;G¼PíX@´\®T@ƒ¦Mà?ÌûWϟ»?Ìs¾ÿÖ¤@öU&£ø@Dz"ø?í]ì_9K{¿Ó¥Üû(¿ã²°â
¡š¿éòÂ?U*¿ìÏ÷>^‡¿ïØÎÎ.̜UNASNone?托P…'?¼"!ý3{?‹Iô^ÄØù?€˜МÓÉ?Ò»ïQS?¼7Á©p?ⶮÜæ?ÁÇ͋°ð?© ߛ÷æÙ?¢eÞ'Ô_‡?×o¶®t¿g?ÀI+Ci{?çÏÄoÊ×ï?®§ãÊq&?£N'ò†Õ?"1Bޛ?ËíI™üëÎ?«Üå~†¦?ãí+n"ð? ÒÆþ*¨?«÷l†Ü•§?"x?ÙÁN?Ô¦»'Í-¬?Ÿ…lè?׈']¸£?À«¦G¹
c?›làz
[?' ç_Õf?ã`OÑN'³?Àæ>|¬<Î?Ò¦¤óù?¿øIÂå?¸_üP.R?µz«—Èß?ã«ì­ñH
?À]©å}Y?ÝÀ…
T'?µªÒJ©á)?´ã-tGô? )ÿý­"—?ݯ˜DÁ?´R䌛ª!?Ô[nôˆP?¤§U"ê°?¸Ê#ṄQ?™¶dÔ¶"4?â¹Ô­þ?¥‰çEÈ,MIXED4FGL J1741.1-3328¿éšp²Ö½£¿ù]ÄuqÀ9ÞL¸ÒDÀ;;3$º¼@§T ¾'v@$ÖÿU¶?ъ'¥aMù?âjd!èˆ@.;|­Ñ@ÍLVšÁb?Ü3ÿ`óµÅ¿Ì-ü}¦ü¿âԃ ±¿àIÓpóˆ¿ïÿý¡UûŠ?ïV⚔k\UNASNone?Ñ)\î ?¿Jã pE?Åi·-)+?¼QË[ªí÷?âC)å?ÃÐç£;Ñ?Ö-ÏñðGÑ?Æ9»Ø³µÐ?«5¨3‰q
?§?>Ïá?ã5½ƒ¦	·?Å/«ZG…a?Ö%}$oÌ?±oO	Ûÿ?ƍïAkÛ?ªåš!1‡?ޓ‹M%¢§?²Vî4ŒµÂ?Ô
.&Y*?«}rS{õf?»Jí¾à?šùµ˜e­}?≛ŏ?­•—+€6q?»žœÈöK?±Núav
Ë?ÍÂÂ+wìº?Ã%v֏Ýó?å{òrVg?ĸ
þ‹¶­?¸ýÁ[[n±?´"û.¸cÚ?²uŠó3u?³ÿ¨O솹?ꑧ(mK?¼2nþ-?ÅvDf¥¹?©þ™ìƒT?É!Ѷõ?°˜i§N?äa¦r3èÕ?´+B-^ùY?¶ë©dpv?š/îï²6?ÂïˆÓ<—O?ª]Äa†g??肀VL?®Í%¿ÛŒSOTHER4FGL J1741.3-3357¿îÿ–ú­Ü¿ýÔlƒ¶ÙFÀ9Ä«^½ûyÀ:Ñ¢¡€è@ ¼Ü¥1þ@ø¼þ#@B–³5L?ãõ@‰]@ƒm¨z-@ã·­Uä
?ãÔ<ÞÓj¿îÿð:»?íD8>4ï¿ç.þúG¿ïóZ _†x?ïIÃ}˜²UNASNone?Ùãй/Oé?Í4Ž^õPF?ÑÒÓ	'¦?Ð0éª?ÔI\5Çr?̺Q¢+…â?ÇüNã›xõ?ΨW!¤ë\?° (Ÿ`?¿RhF/$?çüçC'ô0?ÏhЦ£­?ØÜ֓'Ã?´}‰ìɤ?È$bÇÊ?°Œ'kš0W?Û ;tº?³¬\_"tž?ÖÃûõPÆä?Înü(Y?€Öðšbén?¤ieÞC?äZ¦C
(?ÎO"ȁ0?ÕǙ~Ž?ɗn;qñ	?ÙLš''?ÐÔì*©?ÑǛÌYà?Êó® lå?Ä7+o´?ʨg¿Ï/Ë?´©9í‰?ÃÀßc…ê?èeÊý"ÀÂ?ÍTžN{h?ÏË>U-âo?°ŠSfÀŽ?Ïxbᡛ?²÷<ýîJ#?à/'üý?´%®~¯½°?Õweþ?Õïî+?š¸rwÁ®?¾u¥ôpÕ«?äs™‰m@d?ÖJ–áSâMIXED4FGL J1741.5-2344¿æ8?tè'Ú@òÒ»#WÀ9Ê:̄¨qÀ;´w K@3Æ̈́W¾@NˆÄ_@?ÑcáPè?Ý°Dä6@
Ž6A?û.'Å?ß?ÆßÅDd«?áÜlýÚ5ì¿ß±ÔÄ(¿ê[Ы~žl¿ï$ìH"É?ҟ.Äcœ²UNASNone	?ǎÔÆup?¿ÄX´÷ï?´V¢mæ}ò?«6ùàWù?ç'v¬HŒ¦?Áo›V»¬?Ó<==M=v?ěEfø˜¿?É©_0"mÏ?¾spSéÐØ?ßï*¡‹£?Ãx?RŒ{	?Ð{øa®¤K?°•PÕGª?¿GÃ
0j+?¤Ü0ªLª?ãÙm' •?³TÀåwŽc?ÈâÑâÇq)?¢)<ËÏ?ÆRö§¼œÿ?'°àëº9?ä2Ý^üv?© ³¯¾uÑ?´øÎèþë?¬§ÞÚ*?³Ø
f:´–?«è½ÑÙ½?êåäzµË ?µÇ§Ouð-?»B)Šä?¸CìÇq¢?Ôšúþʇ?ÇËýŒ–?â"íQ@~9?dzM°ô?¾DCXx?¢‰çëyDÁ?¿˜/‡é)5?¨ç	ðáØa?è;Q†Ÿ/Ê?±c":idF?¯~j3¨ä?'AŽ¶SÉ?È/^ž¾>?©/²¿î2œ?çüZ±§Wr?­7E·POTHER4FGL J1741.6-3917e?Û`6Oâ[ÀÞÉâ6Á]À6ücÔÀ:cã6îª@~ÇäیX@cyú—á3?˜2™sW;?‹Ë<Sî>·?òV¦4²4@ySÙFí?í¬œuìì'¿Ò¾ku™à¿áÁŸÂ¨†œ¿âCn9œ¿ä;˽Ù¿ÐiÕOçŸUNASNone3FGL J1748.5-3912?ÆÐm@JGø?ÆLTGç™?¡þ¨'ž?§ÁjµSÕ?é;TÆ< (?Éeşºx•?à³ÂËÓ?ÍÜÿ¥ÖÙ?±ø¦üJí?··–+'?ۖžo
Ì>?Ëg£áñø? ĬÓï?©ê'©™?£L®E?~?™tSØd
?êE·l(ü?¬ì—:Á2j?Û.~©º_H?¶Ã‡r³M?·¤	YŽõM? :k%†Úø?Þè~ÿlÅ?·—f–:~&?Ê+@VòÍ?ÉD_SUE4?¡æ6{ù0ê?¥ù<aB*Á?èV̔åø?Íâàí?Òö7=žO?ÍÏÔ$k+?³8•¤=?¿.C—%îI?ääzB'?ÍëÂ'ϟ2?ÀâoB?©x:šÍϖ?šŽº~§¶ú?½Ð=l2ˆ?êóÐ&üø?«Rg%àµ?Ò>€€U›?¸*J@ñ'?ÀîL_E?«É}DEÍ?âބ,Ÿñ"?¼,}êð
MIXED4FGL J1741.6-2730?çIŠL
Žx?÷âCV–åŠÀ9"uÝÒ®ŽÀ:ys›Ùú@ìØwÐÇ@Z5Ö|?Ë[›\<kì?ÚÓPtŒ™×@zÄÂ<P?éB‹êÂk¿ïÿÙÐs?ïÿÅè¬ý$¿æþýÝ;¿ëTGÛ`ä¿ìŽyP¨9¿ïÿgßbP­UNASNone?ÆE-{ä'?ËÇ<:ÔùR?ÓEәo¨/?ÐáKKpt?àËÊÔO"'?Ò>µ)dtÁ?¬¡¹4Öï?¶ÖtsìÆ?ÔT¨H‰Î?È…GìÂz?äJ/ª?ÈÇ1É6üR?ł»"ƒv?ªwF¾˜f?Ë°ôdÌ*?°™§0ŽÛ?ã³<xy?²«Ú9_È?"ÓÅ—?sØ`õÕ?Ô­Î!%—?®E½:R3?å
€Þ¦'Ð?®š†µƒˆu?¿-ÅönÜ­?Ƙý½Z"?ÏÏ:?˸8¥&ÚN?äV
cži?Ыi'ƒI?—­ z—ød?¤Ž/™zÙÉ?Ù¥Þ6Âô?΢ 6?âo§á83?ÎS–#²%›?ºÞlþÃÈ?¡ö. ¥?эñŽçÓ¨?´]äÖýÎ?ãÝ9¦ÍT?´H$`)?uÍÅC4=å?`A¡AÏõI?×$xZY¾?¶ÈöÅ?äÒ9j§5?¶"Ÿ¸ï*OTHER4FGL J1742.0-3020?îòÞúvÔ¿±ƒÙÓ-©À8de+ÓÃÀ9 çJ&"¿@¤_ݶ)@ùGÏ¢j#?åãM"M2?Ò'5ø	'@ĸF-
û?þ FnÏ@š?éñUbˆ
{¿ÕAuÁ"I¬¿è±ÿ÷œ"0¿çù΍—,Ø¿ê«-u"›¿Ò¸`Jã(UNASNone?Ÿ÷þÞ¯?¡J¿&R|?ñ°Bè±Ô?Œ6ãÇò5?î¸yMôªŒ?¤EJ†è»6?¾ˆLElµ?¹núO£¤?­Cí'¦±1?©ÍƆ‡z%?êZ­ƒŽó×?ºà#ÔÌ?¿öÜ»:B?¨w‹ÐùÅ8?Áÿb¶®}V?«2jD^­?çKÑÜùb?±¤óؾîI?Žú ›j¥?…žhبðq?—к¸»,m?Ý0GEŽÕ?îUXþQˆ?•ÉüŒ"П?¡LJl0?¬¦'Æ?"Eñ´ŠL$?¢…S;'P ?îMsúj<?³€R!•9?ªM+Átµý?«ß笔?³šÞGÌ'?²2Ì<Žc¡?ëçрÄ><?µe눕?µý1ËÀbz? ¯:Ï5'?Å,õ¡­9_?²lçÙ?çõ]ój	?´)\¼5Ô7?'*…a>¹m?s"ÄÙ¹ôF?Õ]줖h?•XR…©?ï8rŸ7q?•Ÿ"+u<OTHER4FGL J1742.5-2833¿Ð!¢ä¾Rƒ?èÃoõPÀ8Â.jÑÀ:"P\8æ@i.r.E¹@(¤~Ïé¸?É@h:{üÑ?Õã*Ý#\&@qìb"IÏ?údDÊ=Ñ?é"L["e†¿Üaq¦3[¿ãONâ'/=¿èÄ1Bm7ç¿ï;_A"Û?ÑÂìúUNASNone?©) Øà?©xÐÿ¿ñÑ?±!{áë?²P*·½Ô?ìI7ÿý"?¸í¥Ú¹'??¬Ré'óf?²š¡šX¬ ?»½ßýŠ?³àûI`;í?êۈ©?ºƒHZì?·%«cB0?£Ë¿ý²?½=æj'«?¥C'ñ+i?éyÂÖ¡.[?¬Ê¼G²x?höaç=Ì?sˆ5½¼?·dÆ9pö?"x²VD~a?쉴`'³?•GC×rÂ?'DEW·œÆ?"3+–k?«öÞWŠ?¯ûôÕôù?í¶oïRJ?±ïl(¡?˜Ÿp4â? ´Ì¡"öÙ?¼Þ¼ñ.ù4?·(^^ì/Ð?ë£+iÌ]¢?·Í7rV5?®tÏä?•«TXÒ?¼Ïg¢",?§ÂÐgE?ê}E‰é?«	¬jm\?j¢©ÏNË?VÈ~?¼=mN"-?Ÿ.·òÅç?ì]¯³Œ^ô?ŸƒE/º ÛOTHER4FGL J1742.8-2246?ÌÔv?Þx'@
ñqýs]ÆÀ9°(¼·«ÓÀ;"bGóµ@Š•{&çË@;'÷
è÷?Ðl8¢Þ¼¹?ÛþÍzò@Ã#·;k@G91úÎé?ì«ÊÅ㤿á˜Tà'^¿â[óEÝYã¿ê*€Â2?¿îfd¸ç<»¿ï¸àâ"UNASNone?¸5Lÿ<U?°ÂÊ1ÀV?Á`Ë@t~?¶3Öå2&÷?褦†½Ÿ?½oQ,êÅ?ÙSÀ‹9É?Â\#íEY?¾€€|A?°êޟùŒ?ßYLpç&?Á›gžl4?ÒªÑë¾î?±Æ{IX?Â÷ù–"fW?§¤QCïŒù?á오Òó?³þÓï8¯	?ÌòO.Lªº?¢)©²ñxa?¹j&Ï´?ö†0ݎ?å ~ï¸ùË?¥´¦Ë'W^?¥a'Ù@`‰?–¦ßìþà4?¹äïìC?±© N*åš?ëmeÔE<?´b ¥Í3?ÃޑŒ@%ñ?¾GÂêÔR[?ÈPl‰¦?Àš
z#Ôé?äô[BW#¹?Ä~Ù=¸6?ÂjMNšöD?¤AYA³Ö;?Ãê;C^4Ð?®	Ž"ÅÙÅ?æjÝÚøDÜ?²ºÞ#_?³ØZ{âԕ?•ʃ1ÓV?ºÚˆæݳê?WœI!\?ê)£"~³ ?¤2qIçbOTHER4FGL J1743.0-3201?ßfÈäi.¿òlÛzåylÀ8òñÝ'ŽÀ:i›€#¦Î@;MÄ®ñ@e|áÒîO?ÎÔ6SÏ
?Ñ!Œ!‹ëÜ@2€l'Ð@¤æ'™ð׿ïèùôMDV?ï,™†Nc:¿å!"dƒã¿æ1Iï7Zà¿ç~Ê-ëÌ¿ïÿþøþ"UNASNone?Ë0¨Çè?¹¼Ù\±=?¡Pԉu-?¢×'vu"?ê&Õ6¨³"?½ãÅ6ÖUã?ÈH þÛÆB?ÁB¤¦y75?´d̾å!?­Ã
GªÚ!?ça^(C.î?Á6"YÇO=?ÅÖ'@®o?«ù›vŽ]Ä?ÂÊ܅…6?©DUAìW®?å׿ü¥¶?±fý	9?À®@zn†?™
‹Bj"?µU!>,û%?'´õëˆ?é)˹ãwD? püýäi?Á[?/¯‰à?µÌ)…§?WA9èÊ?ž+°Ìª×É?ê¾v+ð²?¹Æ>ÂwM-?± Óc¯?°AA3Žé?¼¤.óÞ^›?¸ºÐãí,?êGw±Îæ?»¨KZ"Á¶?»pGCió?¢ðšÈ6P?ÁìÜé
×0?ª":fø?è¿ÝP'¶?¯é 
¾8ó?¨!UÁü°?ŒéúºXÇf?·ŸQWu,´?œÙӊE¬?ë‹c¿~@ß? ¶ˆúC[OTHER4FGL J1743.1-3049c?ïùÃy֟x¿á"<5:tpÀ8®XŸÔF>À9ô"Ÿ^Õx@—'Ýè¨ö@@Ëò¤Î?ÊÈË5rþz?Лüà»Â@éý_;Ð@Ðyí¬Á?¿ïÒü›K ?ï½pŸM8¿çh*á«I¿ã'™îLÏ¿èõ¿¿óö\¿ïü\§ ÃZUNASNone1?´x
ËÎ'É?²ýÕ1ƒ?šˆn€•I?šÊÅœl4?윺Õö¹}?µONo?L?ŶÿIælË?Á<f^iþÝ?¶¤"*µ?±Ô9Ÿ"@«?ç½»ìøÛ?ÁD8Z?¸÷ÿ‰Ž?ª(ggÃ2Å?Ä-¶ðJ3?«ÖþÞç¼?æFTƒmÛ?±8§ú>ý?³M)¦Ýóè?˜l"!](í?­†PÀ3?'SIɺ®?ë½ú–"…€?¡Lëëöޙ?£<o*±ä§?¯.G\@?œ<"]1D?™Ž˜ð¸uŽ?íêWú4[t?±–{Ôcy?°n™¸8Æ9?±:v±8ý?Â+ì1?Àì1ƒ¨
?ég<!™WÕ?ÁÉWy…õD?¼Z¨J¿õW?¢èwF_?>?IJ9ÿç<¡?­S£F¯?çHw7¢Œ?°?>1e"	?šÖä.¼v«?ˆ¼ÏK#·7?²AO·''ú?j©–Gó?ìáç²è[?¢+"÷ßq«OTHER4FGL J1743.4-3123?ì_&óû:¿ëú¾ï>'À8â֕£jÔÀ:@±NÂó@ 4^lFû@Ú½]Äu?ñ)ŸÖÊ|?ÎÕ< ˜@D¿ÒéF€@ßÿtißB¿×ù\B 6?ãsʒ`¿æ^B.ù"¿å#•0~M
¿ä{õO¡S¿ìä"CÆÿ-UNASNone?±?SÆqV?ª€«Ëb|?Š!P´WÈÚ?s?íoD—oÚ?­U
V?ÊàÄ?NcT?È3±thˆ?¥Ç¥EŸF'?©ºð8Y/>?çëT›ÒrÃ?ÇAÆԐ: ?Ä îž??©®ÃMLX?Â÷[Î×?­
ÃÕ/Üa?æ9í'éL	?²!ßµÈÿW?ɼM|þê?ªú˜s:"?ŠlaŠÛüñ?ˆ¬f9— ?é';2''â?¬I§ŠeL ?­¼j'ç?¢¿÷êAX¹?‡Ù¢\܅ð?‹y*b?íÎí¯¬'ª?¥ÊùäÒ?¼"Š¡Y+•?¿1p<y?°³ÛLJ?·ws§]Â?êW-¨§ ?Á}&œKû?½ÕŠ¢°Å?¤Aœšj?ÃÇçÆß^?¯Æ4LûÀ²?çel"¹ò?²(x¡Õ¼Û?¹é9:Å_?­öÇØRYB?'ê$â<?"Ø!Z;âd?ìw0_æ'ç?¯3}‰WROTHER4FGL J1743.4-3406¿î_pö.½ÀlZßI§À:ZKÄ#°ßÀ;®
9>åï@áÑcµ\@Â=&Ñü?Øéq}ñg?ãÜ|m8è@y‡Æ2~Ø?óï•!îZ¿è$EÅ.î?ãü`£®ÆR¿Ï|èˆêö¿åÍ´Þïd&¿êŸÐJ/Îû¿å¾§°³'UNASNone?ÅSº@œìú?¹~ˆÒ§ N?ÙERÐ1†?ÉÙÌåvfå?܍ô8»?ÈE¤é­?Å;j­PŽ@?Á‡¯Ø?ÁòÉOƒ±?ºH…¯Îý?æ4sÊø"?ÀðIøÒu?Õæµý¹ê?±þ9º?Éj‡ƒþö?­ðˆBù¹?Ýd@G)?±å™m~ýo?»fw¿elR?•#öð°Ù\?×´KØVÔß?¯O~ôJìÃ?à¹çè?¯¢£•?¶*'ù¼—?«¬¥˜‰ù?×û'¾qüX?Æ¢"'Á±?á<ù¡}Nñ?Ƥ`°L—?¨°qaý?¬€ì'¨›?ÄWWcå-?ÁZ…è?é_#%î•?Á%±Ñ"þ"?Êi&à¦?«rËX	€?ÐÙs°À–?´a—t¦E$?á¡|ošË?´ðAšIÛ?žà6	r?'ru9OCj?֓yûªÁñ?»½gµEò?ãÆ,±M7?»¢É6Gî4OTHER4FGL J1743.4-2406¿çÛyoÏé@yߖÓìÀ9¢"'¡WÔÀ:èñ«©f–@ê£q^¼ú@Aë¾íç?Ê{‰¹&Ò¨?Ïe7ýO1@EÇ
âA?ÿNç àö%?íQŸ?ûs¿çzä7Lh¿èZ<ŒxHç¿à"à4ˆÉ¿ïÿþøþ"?ã8}àU•´UNASNone?×k@]ñ«\?Ç*%3ɺ?¬ïԆüõ9?¤‰Ïïcr
?â{bˆ¥n?Çgôúq?ák$¯Pª?Ç߃."^?°;I
ÅMm?«>ÚI?ÙsŽq?Å­†¯öÂ?Ü.æ¼{à?³¥¢d)y?¿
§} ÖÔ?¥Úsk?Üod;é»?²¢Ø$ÍGz?ÑÝ´u+êÙ?°¯Qéa?ªæ®)±oÈ?Œšáƒý?åbºâêpw?±%Ě*6€?ÐþاeN?¿d"È´º?²4§pí‰ù?ªR†, ç¤?å¬k¥·×j?Ál»Æ{`/?ͯhù=Ä?Ä옾—Ð?À`ÿ"uBw?À<{2®t?ä{åܓ>a?Ç^EÐÄ©?Ðü–p'¯ã?­®½Þ–z‹?Â*Ræúÿ?¨ŒýÍiG?â÷ 
ø¢O?±ª^Ô²Ûp?µÇoS¤®? ±ìü·	?²$¤)^?ž¬qw6yV?ê÷-‡çYZ?«•X´°MIXED4FGL J1743.6-3341¿èåxÑ^=ÀÝ!ê6À9•$Š#À;‰¾ZCB@ m™Y_@õ~íEé?è&ûíKÈU?È/«©¼|s@øZðŸ@[2\sž]?ÁHç$'Ú³?ènæ4'¿Ëñ.Uþº0¿ä5çéóN¿ævñ~\ý1¿éIO4¹ÀUNASNone?Ò|"ôvèr?Äý¶ÜlõC?‹'ß'8ÿ?…¨¶‹ûré?æU	#6³?Å8ÿ¥ÎA?ۉµ3[ª©?ÌÙ˟…?'§Ìd(]?•½ŒB7ç?á­çª†H?ËbãÏóÇ?ߘŸuÈüU?´ì¸:ô'›?­oùšÀÂ?œ™ÿR؀d?ܹaW€;ò?´1SGa?Þpĸ'?®Óèv±Z?Žé¿q¦}±?'Lh͗¢œ?àKö¦:ó?®ÉÃXVo?Ä[&Œ†¶"?·ç†?'ýÃ_œºå?'p…½7Œ?êQHBA¡"?¸¨¯j1O?ÊèJ¿õVŒ?ÃAOëû'0?" Ö<D?œýdÝ3Ô?è¤ìÐð•K?ÂàJ@s–-?ÐÉe…|…?±%…ÕÕP?¸FjÍr?¤çš…1?¯?ä'ù¬Ì?²…
 0r?рr·é¢?¶ÐÑ"εP?†mK"ŒI?e¨ó¡b?æçÄïL˜N?·»a™èMIXED4FGL J1743.7-4321¿Ó2? ÝcQÀª#žj¹²À9ËÍiª¾…À;òHv'VÕ@äÖÈN7ñ@^½$¹?Á–I˜z_Ã?ádv6¾/@9ßÞè@Ž÷Õ:?豈bîпšàRe¨{_¿ÞƧCÑ;¿éûß¿˜±½¿ïցz"ð¿í¤{	‹™ýUNASNone?½(}]ßë?´QFÎÙ\÷?ç#Lç…?Ä*I÷è%æ?Ī¸$õõ?º(‹W•â?µÔМþ'?¶x½¢õ?àÃÅË6?Ä1!ð@+?ÙA´¼pð?߀<À›?Ë`†äœ]?°‡3río?ãS's­Õ?´Ž"ö'±?ÇQp͔ë+?ª\ªžü9_?ÓTù¶ÿ? Š‹§{?ÜÖE#(³?¥Y1n"Ú´?Ϫs™Þ@›?Ÿ?jê}¹t?¤i¨'n‡?—ÀÀhÕh?èB[ÎC*³?ÀdÿÅ-Ø<?ÉÜ&¥
ô"?½ñtCk?¦[3'Ù°?«ž'.™°?â'­ä)_Ë?É\šÕÙ»É?Øå=Å;«?ÈÜýfȋõ?µc¯Ü3ï‡?¢îEXÔÌ?ç8©:‡¡†?³—ßGÍ?Èkƒ(5u¥?¯i
-R?¼«¼Å1?•mvhee?âStqÊ{A?¯"*…r?Ô.(y½9?ªï¥ˆÈãuPSR4FGL J1743.8-3143?è#5½¦Œ¿ò:øúRAÀ9['IWbÀ: ¼X
ƒ@!]úŒÎ…	@Õ¼{`É?É2ØÅS†»?Ÿ!N%Ê6g?ße)ÛÃP@Uvꚿí!ñÂO›I¿ž-QûRú¬?è'_³Ä¾¿å'§¢pØ°¿è<Èk.L¿À•¸#®UNASNone?ÂcsÊß?³oÞ×*?"µ9YÔ6í? ±¥=·|¡?ë''="ÅÍ?µYþLl?Î$«	r^[?Êü@¸ç ?Š;"ðˆ7?'»&©"j«?è
æH?ʱ´@lŠJ?Î,¹þ?¯× ÿ;û?³'%€ÄÁ?¢Ô
Ê,‹.?æó
B!§?±Ã†ÇU?Ô,eî5A?±±²Dï?…vøù´3?wœmÄá"X?å"W-8rb?±ÛrzK?²â—ŒQœ%?§ˆXRÍ8u?‹kΘŠí?¨¿Òw}¶?í5ýÓÞl?°¶VätP?ƃ8TìQ´?Ã^sCÕ¨û?"Nðç½k?"V@øor<?ê
ö(Ìä?Ã`»ô[?ÁJÞåAýj?¥štíµ#?²ùÃd&Ö?¤KLdʔj?éNÚ'{?­È·Ðy?Ä"¨c-nE?­ŒÎ-j´c?‡Åäø¨øÑ?"×I.pvx?ê˜>SˆúK?®OÏ~ƒOTHER4FGL J1743.9-3539¿ã%—ԝ{¦À	¥%1À9Í:óñÔÄÀ;bʤÔ`?@1¡¸¡ó@‰ÂÁ±Ø?χ?ÏÏ?ä	pA0¡Þ@+vö×bR?ûç­ôDŠô¿ëÝâ¾ü˜?ï2«M÷¿éÂ!øù&¿é©yámm¿ïüpßFI¿è!8>µÈNUNASNone?à.Ô^'…Ï?ºk)«?°HŸ¾z8P?¦—×X´%?ې/SÜî?ÂI!É ¿Ë?Ã[À×1f?¿µL'Iñ?ÐvŠAH0?ÂHr=<Õ?ã#ï&¦?Áð¾TË«?ÚøCÃà?²ñ#Ô|‹Å?·­0ZëÛ? lƛƒŸ?àÝå×he?³œõÍw?Äu,Û]è?™tõê5:
?ߖæ?©ßOOMt?Öe©zë·&?¥Ú¡ü³}?ˇÕjä.?¹*rIêI?¼YÛ[¹lÑ?³Ð§2?Šˆ?å'Ï:ÙZ?À`ë® ?¬m†øút?²Îúˆ¥•?ÑÞQl%?ÇîðäP™?åJçŸêt?ÇÎÑ/™0ú?ÉÃ3ѓ°÷?¬X'ãþßÈ?º9"ZÌe…?£Dtš£Þ+?æH A‡?±ÒËL@¶¯?¥B7™/£?‡\ž®¯¿ñ?ãvÍ|ӘÌ?±~¦é?G‰?Öo|¿ïÒ?°m@×úMIXED4FGL J1744.0-2504¿ïù§—šL-@ƒá†˜5À9BÍl.ýDÀ:¨ÙRîº@¦9kÜr@§"~§¥Ì?ÌÓ÷8†.X?Í>@,•à@²Å"Ùîô?ð±BøΊ?êÑr¹[¿ç¡ŒâÑñпèÉaÔ¿èç¤T¿¿éñþë-
$¿ðUNASNone3FGL J1744.5-2506?ÉÝtÖ§Ó?ÄúØθµ?¶|
ÁAzà?¶¹+ìÁ)™?濖êxë_?Æ?dœMµ?Ò¹IÊ4¨?ÉD¿žLB	?Á2åvxœ?»wyý$¶÷?âV¼|óp¦?ǘ˜ P?×=²i/±?²ÿ[b5Ü?Ã1Ãÿ@3ï?©›B®Âm?ß)k—0fX?³'•ý(y?®Y\|R—ð?TÜ;¯Íp?¹ý¢hÜH§?—%ÐGvNJ?êÚµëVG,?ŸEp!¦?ÁñÂÌ)?Ã?DT~î"?³K% ِì?²bÓgy?é*¨öü?ňXº½fä?¸ÝÅjô8Î?»êmÑó0?Ç
Onþ?Ä7ø Úã]?ç!³wîÂ?ƕp}t'£?ξ0è*KX?­ÑR—Ô'?ƕõé._í?¬½Aß[`?âªöK dÏ?²õêíé	ì?'¶¯þ+?vÿÝi&Þ?»óW÷žî©? ÍιÛÃ?ì˜ë›ù?¡·v	­¹óOTHER4FGL J1744.0-1311?æïÐ!ëã@ çqdÇ)öÀ9®ù–Ys9À;Tpš@(żãÊ@íqåöi~?À‡kŸ‹K?Ñ"ÌHBŽñ@PLýߔP@‹È>?ïÿº*2Ùq¿À¿1ÄPÉ¿àÖŸd´µ¿áê2¾™-c¿ëÃé.,c5¿ïÿŲýîUNASNone3FGL J1743.9-1310?ÂË+z?³³¿ëY?ÁY\aC«•?³'Í£F¹?æöãœÐŽV?½ŒÛ4?ÚÃÖ¸g?ƖžÁ»e‹?É}]ó?/?ºÏO!êû%?Ù/ç‰¼'?Äv
Ä ?Û=hJ •?±µÏBQ?ÌO!N6øB?­ë''8?֛ßcJ?°dsV•·-?ào7¢Gä?£ƒ€ýC?ÂÌ»Qq¯?"OÈj<Š?Õ»3Ëo?£]%)m'D?«âçÆA?¡;|æ'ô?ÉڟlÜ&?½R¼ÌŠÃÏ?çË)³quÓ?¿ÿøÚXì?ÉáÁþŠ—?Á7´2ˆO?Ò®ô·Cðè?ė¬Sy×?à0$»‡f?È¡@ÏJwë?Ðw?°1u×%Hí?ÒÜÑ.RÆ?³|SS'z?Ý	¼—ÂÌ?³í­¼?Ñveó5?¥nñ;¡S¾?ÌöÆ»ù?¦«~èK*?àC¶@Ì×g?°}8¿–ÛMIXED4FGL J1744.7-1557?ˆ>͔J@Ÿ§¨PÂÀ9ybA=·ñÀ;m§<ð@"ᷕƒ@ìC9+?½º›ÇÇ)u?ÏõðÝx@®@Îގ–0?übE1¸^×?ïÏXBaNz¿ÝqÍbHõg¿æ(Æ}}YG¿â£Å&p­¿íPA`ó`¿í±P$QïUNASNone3FGL J1744.8-1557?ÃBù!Èo?´)ZFÿ` ?ÈZô5zô?Äóû°&ä?å"ª/z'?ħÈ2d?ʳ¿à€2ë?¿%!UBÛ%?ÖuJqþ?¿u³åŽÿQ?Ü0Å/t?©û¬ön?ßøþs?±Î"â7§"?Ǐ±4&3'?«Š­Ìå?Õ6.Ôîs*?¯¡72hu?ÑåDŒiõ?³âd…?Ñòñ9=¹I?žˆ$ôà?Ü'Ê»5ÜÂ?¡m"íˆ:>?§ïÇlž`i?œèõ|R
?ÎK—Q¯Žè?ÀÌ)Œžçë?æî´"<€?ÁÀÄápó³?²p&³¼é'?°eÊ选>?Ük»"?ǼX3Pm?ßF‹RŒe?Ç×Ïj¢?Ò0Œ]N˜G?°¸º= kè?Ð'¼JQ:Ž?±ÓøäMŠ?ݧ·X`-+?³._ˆj‹ÿ?¸‡!²H?¬êmíOk?ØT¿p©òh?«B˞ÒÓ?àļ&P:š?«Ä
pò0ŠMIXED4FGL J1744.9-3322¿ÚåN¢¿!ÀÎú¤vlÀ9x ]Øù+À;!ÖÜñ?@ES#há@Nc¥ÁÆ	?Æe
›º[0?ÝĄ^žò@ÞÔI˜Ð?þ§/ç¤>Ž?î&mó"¡ë¿äu°»õ4¿×Yӟпèi¢#¿ìpâ ôÈ¿ïôè_Op×UNASNone?ªÛ]n§ã?¢Þø`ˆÝ³?Ûo²Sézò?ã¾åÈ5'?àšpÿy?ÃZÀjé­Ù?ÂÈéFÔ¾?¾Š<¼@Z?Äá³0:þ?¸~øàÜ?æL
A±ü?¿È­g4u?ċ‡r¥Žð?¨b(:È,?ÐA» ­A?±'šÂ—o?â¼@ŸFE£?²Æ1Ý4Þ?²öÉËӍ?‰(ŸèZuV?ÐèÛÚ‡`?¡sԔë­?å,¸ÙŒ	?¢J*ZAv	?›hÍ#'Û
?ŠÉ'¯?Øʺ¯¥î?É÷k˜½?â¿\>øÁÑ?Ót=¶ç*?¥Ý¡ç^?§žî«	|­?Åy}\§
?¿ÚLZT<÷?éCƊ­1k?À%L=£Ø?´Z,¥E6z?™˜øx»íE?ÐEüªq>m?¶R˜±Å¾?åQ¼,xj?¶X¹¬=óò?'<£wÓq
?sfÊ?Ó.žÃO ?©á¡ÄVÓ?å׶˜?©Ã¸	ÈàíOTHER4FGL J1744.9-2153?î#œ´£'ž@_j^B«vÀ9•
ÿÀ;o#¤I÷@0–¤Ç @DeÀN9I?ÐҋÿH?ϒ¤g"@í¶^Ì>2@GºÔ§¸¿ënM?ùÀ ?ëÑÇ]w)'¿âü¯þàÆ)¿èêÂKiŠÞ¿æa@AŽ•¯¿æžë/ŽcUNASNone?á
°¿ûØÿ?Ç
a5'¡c?–a'F®ÊŠ?Œ4Àë±Ù?Ü~†[äz?ÆæGK‡×"?Ü&ž±?ÅôA°hW?¹?	ûudƒ?·¹"Tvvj?݉Ÿg/+?ÃXm‡öb?Ûý8´kEã?´%'œæyH?³²ÍįÍ? jÅƞ4‰?ßٌßÞ?³›—Xá=~?ÞÃäZKê©?£læFì/?µ¨Nypë?'\'¼²ß?Ûö1'¹?£ÉYûžò?Ö±¹µüã?ÀéfzL;1?¢…¼×‡?•y
•Ë§à?ã~Ǭ㉎?Á«t
q{¡?ÉxØîW?À:dÈàÌ?ŎËASÔ¶?ÁØ°I£%ù?ä>+¯u?Ãâ«l'	?Íö›
ž4o?®žÛLDç?¸'2öÆp?¡'Ž¬ë?å}rÝÿ5f?±·r¯ùA?ΐ˜»Î?¤«ò=)?»û€XCÒ¬?£@ nŸðÌ?äùkó‡æX?©[‹ŠôâMIXED4FGL J1745.3+2338¿âëaÀíÏ@8~
"¾@BÀ:T3‹GÇ?À<*»êý9|@Mheïóî@`êžnëp?»
míq¼¿·&¨
u¤È?÷¸)W^Í?üàcR4ֿ°£?4É¿åmbÙéë¿ìŠtBrq¿å™Þ"Û¿è;?Á¶ï?âÊC…ÎUNASNone2FGL J1746.0+2316?ï"&íÌîþ?$]{‡ë?qY¥ß2`?q<ŸGÍVÝ?†Iq"ì‡?‰g x0?îï
¸¦á<?¨‹eTf¶M?‡¤g¿1?–Œ6áfØi?–"Ú!†þÛ?ž¸iŸq?íÖùä‡ÿh?žGê7\[Í?³­æŠ?Šçq¾´0I?ªÍtȖì?šPÀYC_ž?ï"}¹\~?{Ïý"IŸ?|e'¸ù?eMŠÕ5?"«¯²â?uù½²±Ð>?ʟöÖ?¤pSšÉÕ?'î»ñ—¸?"c3½-Ô?˜¼ÊÁÇŃ?ž¸0ñõ?í,³µ¥i?·ó8y´a?g4¹èeý?¯§v®¶uî?®4µù¨v?«háVKÛ?ìl»/—A?£îÜJ¦éÐ?œ-Ðû?"öõí>?µv_Æ5Å9? î†«·Eª?ìÇeè¼ö? 7˜]."M?œu,ÑÔ?Ž'ûcaM?²§‹ûšl]?™VFú›åAGN4FGL J1745.5-2249?Þ÷t¡ù §@	šxš:À9ÙéðÀ:³m—³Œ@_#·SÊ@P:ÅΫÊ?Óµ^>J?à™ØZiÙ@	z™ÄaÄ@@d"µÔ㝿ï·]d_%*?ïñ"Á"g¿ëMa²¢¿ð?ïÿû-2h2¿ïí}±«´UNASNone3FGL J1744.7-2252?åx†9žý?Êwù}!?°`Ä웯?´ÐëßDp?Ðöó\-¨Z?Èd4¤D?áƏl!ÄÔ?ÐT¦¹pø?¨½.éb?±qÚxÉú¼?ÙrɁúÒ«?ÍÎ)ù΍—?ÖÉlÿÜ?´)Çü7ÜV?Éxq~¦ä?²¤ü' ú-?ÜzÆÔ©ÿ²?µ
6v ?ä߶?À Ùz–Z[?€Ç)"LÖÔ?€Ó5è1f±?×Oœ÷XLÙ?¿ñÙGj³ä?ã–ôÿj•?ÊeéÇb?À¹&>z†{?½MÂÒ3OI?Ðu"ßÖÈW?Æ£&ÏS:?Õ0"ã¬?Í‰Ö ;<u?½½Vô>¼å?ÅÝF +Ð?á¹¼×·6Ž?̹Hv}|?Ðk¥N+)?±O¨ÔÝÙ?ϸ墏?+?¸¨ƒv&)?ß·è-j5B?·' iF?ÒÕö7vA?ÃÄŸä6?™ÖîAo>°?¡2}ì×?åÆMr,Jê?Ã)ÑëD²MIXED4FGL J1745.6-3626¿ÄŒÛŒ…TÀA&:ý,À9Y©mL3µÀ;KkÊSuÉ@}Š/™J¿@|­€k`?Ŧd׍?Òåí/Bä@…»¾‡¬?ÿ¡?¸§¦Î?ï¤Î(™Ò¿éšÌ¿¶¹»¿ã¥@@âÉ8¿ânøÁG]¿ï¡‰R#¹?ãJò|‰¾UNASNone?Î«î'?¼š‹(ŠH?•üˆwz	?ŠÖ9Ü:k?ç"zšó-V?½‰5wŸãy?Þ7¢úÒÐ?ŀËâ—z?ªµ¼êL?§E]mž‡ù?Þq¥g`¿ç?Ä@k0‹Ê4?ß^Y!Yl?°ðqÜÃ
Q?¸µŸwRh? «¡hvà'?ÚtcöZËå?°6€˜jª?Þp3[nˆ?¨ºÓ»~pÉ?¸97'v;o?'Qv*?ہ~ÀOeï?¨"Óz÷ÿ?¶?ÉUµCb?«cÅlG™?¢+´ˆº!š?—©‰.Ú?ìKŒxýJ?°ëBŸûº?Æ\SŸÜ¡#?¿†nïvðÍ?´…"ø áÃ?´h‹]˜kÚ?çØ8™W2?Â÷Ìæß?Τ';ç?­)t©±?½±s½T?£?\F]û?ä ÇÚ¹cR?±ŸÕWfÂ?ÉdùI,™¼?¤›ÏDfÛ?®·Ðˆ»r?¢äe4Ë?äû¹'ª´?¬a™€¢°LMIXED4FGL J1745.6-3145?ë`U8ÒÀ"¿÷¨Ã ¢7À9·k;¸=À:׆¾Ë'J@‹øyMô«@Qw~¼ž?Í7•˜ƒ%?ÙjÈ˶L@7Lg"t@mºB±€?çÇ_¥'(¿á£tä®k¿â(Ùþc´¿å\ƒÄE>ο煇"Ý—ö¿ïÿÓà<k@UNASNone?ÐmûÿD?ÀÝ}Û3S?¾0É¡t.{?µ)úFÏë?ä]ÎDú?Â×Ø=Š?ÒÝ*ÊÑAs?Å­9'%?©µà&?£º£¨±Ò…?äÿÚYŽwä?ÄBɏfËø?Ó=˜Iëäô?°ýkãXÖ?¾yˆd	Œ=?¥g×ÏÒ?â'ΈÛÿ?²Œ§ÑgQ£?Èhþ&,"?ž×¶8Jo?·ÉØ°î?'4XM]§?ç‡;žÍ?¡Å"µÛq?Ä-óùa€N?³6 'Y©ö?¾¤¼ýÏ?´;ƊÕ?ç"Žj'nR?¼"êjë ?¹˜Š
Ôq?´s±Ñ¿gï?±`A\Iþ?®s(fÌI?ê æže~?¸*n'˜
?Ě*;Îô?¦ogt‹ö¡?½9Ø°ƒ&?¥ë"s{'?ç2B4$l=?°¦ÉÊz?«É+?6?ŽûiEÓo?¼Ê¾Þ*Jà?žHUNþû$?êªQ¯þ"? ðQµusOTHER4FGL J1745.8-3028e?ëŽÂiá4¿êÈè§æ›À6ŒŽž"Ô^À9¡PþU0@ lÒ³k§Ä@æJ>ès? kæ­ôo~?˜ëã=|?õ×??ñ/Q|I}?ïIše]R¿à
Õç'Áæ¿â#揲¿å$;´4ç¿âÀœ<âž¿ÝŽèÑQ­UNASNone3FGL J1745.1-3011?{Z)ÿø?‹‰Q_߇¼?p¨Ü9ʤ›? B»ˆ{?留'ûç?¡·qF.Ý?¢ä¸Ð]¼?®W™1U=?ÐÄ
òÞj•?Å݂:
"?æo®ùþY?ÅðÉ6d?­Nú#"??žÔŠ$ihe?²ßöüõTC?£®m;AÊ?ëÏH#t?¨ÞBe=R?™mã®Ï?"¨¶aU$?¿ŸRý97j?§¨¶'"Üâ?ëC*1Vå?©Ë³¼îMõ?'ûM°æPý?',qú£ˆ?|Ax/J?¦ó©êÑmç?ï{¢$,°?¨}b¶–p?˜þØ	WFØ?¤oÞ9z­Ã?ËdÜOÄô?ÈÜë={5«?è^Ò+íÜ?Ȗã=ÉÜz?¬(V…:?›™B]|ð²?­¤>Ø믊? i-®'	?ìc:ÌÑ÷¦?¥S|ý?…pQ÷™?vã{s?ÃP$®h¼5?±,˜'«J?êÖ5Œ‡jö?±œˆjÛOTHER4FGL J1746.1-2541¿îŽÖOµþ]?ùMë­òíÀ91áìï'À:ö"o³í@n‰šs@1*å†×ö?г ž†~?Ñ!
Gé#@
MFðP?è
ۉº9³?ï±K(¿åV…í	¿åǐbcL¿ç§/^½O¬¿ë!¿îB¿ðUNASNone?Ø×@#¾†?ËÊi<¦ñ¾?ÓÇxþ!69?ËÎ꺯¥?ÓaFÞÙA?ɂþþßTË?°'Ì€?·²ùÎùÒÞ?ÀF™ G?½{&k=?éî´Ü¯Þ?Ái	櫳?Ðôä!Áày?°ÞF'Ø?É>¢ä,K?®Î3G]À-?á5å6üü?³Kðŗ§¼?‹Ô'ö*n]?lfj¶¸Ôi?Ã6¥èv:^?¡/0{:?êÃz@Áo?¡Ëšƒžú?ÓØ(h²y˜?Ëyå|ϒ?Ò4ñ?Ê
'&­¶)?Ú
£'%´š?Ì¿LïÐe'?›®.¬.ÕR?¦;«> ?Á]ØdýÒö?Á"ðÞ:D?êËpþ߈?ÁÞ\þCùe?Ķ²?i½?¦î×@qžÏ?͙²l
¥?±ýYë*q?ãkæÕ%z¨?³…%Rb?g]l𫽠?RàqD|?ÄÅrGg•?¬\¢"rŠ?ê·F/ï¡?¬U¦®ÜËMIXED4FGL J1746.5-2019?×ùG%û´Ž@._¢ýÆjÀ9l~|áœÀ:Ø¢xelk@µètž›@.ƒþý¡?ÒVñé¼Çœ?іé;ƒ)@	±ÕšÑ§þ@€¹xÝ?á7¢~D©}¿¿K¾ß8¿êTݧæcw¿å›ã@+¿!¿èSZ_òÙÒ¿æìa¢—oUNASNone?名®vAó?ñ?)ØãÔ?°_›4{+?¯‰"«Ý®?ÐÆýÖì®?Â7Št¼ã?ß¼†=Ç5ß?Å÷×ÃÜõJ?µŽ xMG?²ñÑ0Õ??ÛÖöÎ?ÂÕù§Ýe?àÝü(¹?´ˆC¨BÌ?º€J	°Ð9?¦ÍŸô?Ø\3M›z?²gԛ?فFd/?¥Ë£Žx?²?m¯K?ŽŠë5,l?à÷{K¾h?¤ã²Äó@}?áoWѯ÷?Å(O-?¾p—Ïat?¹˜SðÙKª?ՅKøë¨t?ý"7­ä?Ë]1ôĸ?ÁŠQ†c?Å]¨´ÙU?ÁÑ%4u†?ãÑqX¡›Š?Ã~ìr ?ÖSÁ.o:?²ºK\*ë?Áæ´Åo-?¬BIô½B?à~©7l˜?´éª,²¸?Á™gC?Z³Êt?º.ѱ…k?¡"O3­?èSâÄl\?¥8LߘºMIXED4FGL J1747.0-3505¿ïΝöºKÀ³~²†fÀ9;AÖNVÀ:ð~gäì@¨ç ÐH@€"Ýz™ú?Òý¤Ûìû@?àž«QR+@3¡/?ÿ¸†^©X©?î̎^''·¿ÓrP¿á¿ã@Š3Ë	¿ë©Ùîm¿èˆ"#8m¿æ)7fžšŠUNASNone3FGL J1747.0-3506?ľX`f?¿S"Ãõ@g?äqÍ$‹z?É?W¦&'2?Ézs
¾¯~?À´®Âd'Ð?ǀØmÿ'?ÅÝ_adsó?Ѝügš?ÈRe2^Ìê?áØË°íô?ÆÇ
K©1ù?ͦvTx°É?®I0›…?ÓzÒn¢J?°×û*"f?ݱòg!]"?²p-ûSŒ?¡‹Ë
6?'—Ds6‰?Ø%´"9™?°
­id…?âÛ0u=IJ?¯ºæc^ã?©kºŸ^ç?º?|í'hs?âšpÐçRy?È<£zÕ‰?Ñvh€á«›?Ãã‰"2I?«èw{¡0ô?³Njá¿/þ?Õ¹sÕ í?Î0P)ä?ãd¾"ÿÎ?̐ƒlå±?Ã~³S˜È?¨Æ '¬†?ÓÔb3bW?³H½%?á6Gùz#?´Rò6mï*?xõÇ-U?cHo"i?سøPÅP"?»@}¢ÜÓ?ãtI^)?»5ÃcõüMIXED4FGL J1747.6+0324¿îü"J|ü@/{À6âëÀ9®Hn-ÛÀ;¶·»*ä@™Km¼›ý@Λ¤5Õ?½µnryo?Ê0¬O·x@
"­äª9$?ÿlyöf#K?È{ø^v¿â_N_¤¿à©áæ9…]¿ÞZ؍u¿í2wKø¿ïÿ⾦™\UNASNone3FGL J1747.3+0324?àfdHё?À›o…¹h?ΩxùÍ?»TLnª?Ð'cñœ÷?»49æ	?åy
Zöé?Å­}^¿B?Ê[ÎTX¿?¿$lRÛçi?À{¾
 ?·¥x2[?äÕGÐצù?±Ž¡à8Z'?Ç­(d§?¬úž~F11?ŗ3'ˆ÷?§ðÀ»Õ*U?ãDŠË—åÝ?¤'êÅËO?¹Í£Y?'¨,[2½?Ó©Á­Á?¤ÎPúQ<?ÓÍNlʃœ?½U¬²-Ã?ڑK~dž?·Cß¹ö?Ñ¡f|¶´Ý?½Yâ©ê?ÜʧŠ_Â?Ç~cÓd©?Öå)ƒ(‹?ƲÍÙc?È t˜òïe?¼_{æ€R ?ß"²s‡?´åÅ7ÊJ%?ÒÙN»Nö?´tÖ¤Z@?Ìý£7Ø?«Î:û_·?ÖP?X/–ñ?¨ts4ú	{?Å)XHÁdå?¦I;¸[ß?ß'\ÕÞ?±vP}¹ñMIXED4FGL J1747.7-2141?ûä¬+@
½¿cíÀ:ÅÛAÖÀ:õ‹QØ9è@ð_ŸLáÛ@èIåý{?Ô$yÜåɞ?ÀmŸ*R9?ðfÝR@ª¯³…S¿Ð€¡öµT¿èù›ÍP€K¿æöJßø"¼¿ì7ûþé¿Ê$xs'.¿ïõŸŸ1öUNASNone?ã4Ö:Mž?ÈÈɹËá?s!O.\!?oGË£.|@?ٛ™Íà·Õ?Ȳ8¬™Ñx?â]fü%?ÍR9)ó³?™®Ê¥¢ˆÎ?¡*LxF?ÙªE\ð4Ë?Ëñû¾W‹?ã—ž-0?³œ¼æÈÿ?§\@4Ýß?š›¡æo5?ÖßIíðïþ?² ó5Yc?å,Ã:…j–?­ôó9KÆ?p%å£xŒ¤?_ÏñÑ[UP?ÕeáóÇÚÂ?­ñ­`¬?ÕØàÔ§É?Å)¥.¼ð¦?û|8câf?~{Wz=pg?äÌ
žÙ8Z?ÅIx9?Öuy'ÒÈ?É&l2OªÛ?¡"¢l"–0?°¼5Ù^?ã«ù*M9?È?S/°zd?ٗ´ò¯h?³ÙA±B†!?°Ë~'›èB?Ÿàfüq&Ê?áµåns?³›Ëûd¯?ÔI U~a?³`¶ï?éO?}"×Y
?wm¶Œý}'?å &'Jáj?³"›.êÛMIXED4FGL J1747.8-0316¿ê±ü,is@)f+®´À:ÕõbLMÀ<
Ê7Ǫ@!êK¸»?ýÓ
ÔoX?ÓÞõCc'?Ó¬¹1–?ùC,Tò œ?õ`¹ÿÉ¿ïùæuë>¨?íK@š$?è6x—ÁRE?à'՟Ú%¿ç½ûm#D¿ä÷ëÿ—û4UNASNone?ì	|ôƒ†?º:Ä¢ù¿?z0LmPÄH?wà»áQòò?¾Rñ®G?¹¾è˜Ê?î=Ï]:?³TÚkԋô?ŽbÕ[heØ?w°H">™?¨VVÍùî?®$Ìt) ø?ì!líû+ì?¥;YoÎh/?˜	Ü*kl?éç%BΔ?¸ò!†g¬š?¢ÀÃý`âp?èt…`ƒ?²–Z(æ4D?›âb8Ô?‹´ÐX|Ö±?ʱµ§
ÂÙ?²™-q;ý=?ëÏÄ×?ºÎSpъˆ?†×\µÇÿ\?"ãžVáô?ÂoK$Ên?¹×·¿ýäû?ëD'²?Ät
oUßl?¤ÙËéÇB?¶1$äɕK?»r]Eâ?¿8òò¹0?èÌ	|ð/l?¯?.üI¥?¤
'Dþœ/?˜ýçþª¶?ÇÌu{¤ˆ'?«·åQlÉ?ãeiç$fè?Àd¤\½ ?ªðþmIS?ªúR'Pb)?ÕóN—g?Á½,àw"NAGN4FGL J1747.8-3006?ÜÈP©ï/׿ð}'@.Ä9À9ÚZgT£À;‡º.d—@ Îî™Ñ!ñ@$½Ÿ2_Ï?×}Îâћê?ïRú®‡gh@ž–›¸WË@¤öí1Ç"¿ïã%Ô¥ß"?ïgòPµû¿Ø–8ù€Š¿"Ÿ\èä0¿ë¹ýßÒ¿î女©UNASNone?±)Ql/?­WÆó;mâ?›™l'èd?•Pcò?ìþ±wJ©?°£WñI'?¹zòê–<?º«/ï¬?ÑÎBe!º1?ȹE 7k?ã逌­M?È:‡ðú©?Րó#^?²‹ëÉ Í?È_©h™œt?±ulýO
¿?Þ?8FÓ¿?³²2æ³Ýû?ÍÁP7%H?¯U 7ÆÕb?ÝVfì$+?¼",yI†Ë?ÓÈñǔ9ï?µÇM^	?£
|Ô¾"?©&‡"Ž‹×?ª´lÑÚ?¤ž¥s•Ô?í$e¿2Â?±3Dí±#?£>i/49?«sýI^œ,?تê‰÷A?МàLÀ?âv¤(,³¬?Ð^¦³[{?ÈÆS>Á\?¬[z¥¿V?Ï`º}È`_?µø?wê;U?áöL˾7'?¶Ù‰Œ,ßâ?±íˆ{†€…?¤lX ?ãQíKP?Å0ÓcóM?ÔàÃJ~9¨?ÂÁ"šOMIXED4FGL J1747.8-1827¿ïƒì"ß4@æ¢nTqqÀ:Qè·§À;Ê×)G!'@Ÿ6çrÀ@8âºtÛt?×¹vCS;ç?ï.À½të@ß«ºbg@é—M¹ò*¿ïÿ*b{ö?ïûd;¿êPëHD½¿äeÛ&+ã´¿ïÿÿÊPË?ïþá˜á¹UNASNone?À®ñ<?¸Å<3oÀ™?ÛlÂn¤ù?Ë\ÐZËÓ~?܅ÞåÜA?ÊO´Éï	?Õpœ³ˆ
Ú?ËSñĨæê?Õiœ¡iz?LJcª'?Õ&F¯Ö‹¬?Æ/w}²U?Ùé"R#J?±Ï,Í VM?іe‰¾ýy?±ó¥‹ï³?Ԁcîß>?°SÑ9»?ܧ ¼‰Å?²­¦w}®å?ÒuDëlu?²™âÕ!Úñ?Ðã¤s×?®¤þ†!w?±}º,@ª?°K'j–l?Ün­sQl•?ÎNÄÂù?ß1äù'Á?ÎB4|x:h?Âzñ¶™¸+?ÄÒæ)^"?à]@Ó.æ?ÌÀ¤Jwp?Ö~UV°?Ê{wx:+þ?ÑÊã»H7t?°ñpD[…ª?Öo¾Ñž?·[)Ìl?×Æ;øöï?´_jӃVS?Äé_}q£d?«A@HUÀ?ۂ³Õk=?ÀT¬GÏ«?ڍqÃ?½dqÑuöIMIXED4FGL J1747.9-3224?äø]å–û¸ÀÔèÅP׉À:¾¶‰"iÀ;?"øS@+ƒ«›¤·@Ãf½Ì?ÑØýݐêI?Ûnàˆksì@	ÉrŠar@€Ì T‰D?ïðvŠ ØR¿çu5×RaÍ?˜ y
'¿ã5"÷{Í¿êDFwÜ¿ïÿüÚ±'ÞUNASNone?ÑtRßî4?À'+•:m?¥Æ$ ^?¡áx§òÒå?åém½{S¼?Ámš"€{?ٝ2úÂî?ÆAˆi#7Æ?Ã)="V?šœ`'IÀª?âCM9ĜÓ?ż80"=x?ÙùœÍðR'?²Êæà_«Ö?ºZ[;÷
N?£Hû©P"8?ßoÌcê†?²ó,ú¨?ÖÂzìãÌ?§K.°J§?¬õêwë?ŠØIRbè?ã=qfc{?¨~ؒǦ?¼Ó–2ºp?±há'æ?³›;«,?¯—éš|²G?éò%ÙU:?¹q2^V?ŗGåqß@?¼á Õ‰E?£XŠï?¤b&¿÷:?éd­íʯw?½ÃmŠûz?Ê.E>3Ó}?­'¾?¿­2ƯYþ?§÷#~'?å~ÈWá?²höª	h?ÁsÃY?¡s˜"ø?¯úç¾õ'?˜ƒ¹—í›D?é£`­ÈXR?¦'nXóîOTHER4FGL J1748.2-1942¿Öæ½
¯Rá@ålÖÂðÀ9
‹ýáÀ;>–•[$@b'AcL«@-¢ÝåùÄ?ş£†ØL?¿=f<õÔ®?üT\É.²›?úÉ·0Ù;Æ?퍝aûÁ¿àfêþ<¿äSÇÝúœ"¿êHÒ!Š_¿Úý[?Á¶ï¿åës¶±•UNASNone?Ῥî0?Áž\‹B?qk)3H…?h®?
r•?Ü:ùw]?Á¨ºWîî$?ál¡²»?µ<?ÿÒç?¥Áäfqy?¡åZEw›?Úož/ÍÅh?Áj\]V¥Ý?äœðÛ8º ?°á¥yô#-?™Û´Ó#+"?‡pú}¯å(?Õ(bü	âh?°'"vöÕ«?ÝÇE£<ƒ?¤@84'çz?¦,'9•ü@?†BÜtœN?ßs(5ÿt?£Óšÿòª\?ÐàWô]µh?ºë§ÙMc¶?';­BRfÓ?wZ}è¡´,?çFåPÀüy?»X`‹¨a«?Ρ`úäÂ?¿}šcݹÉ?´2c*°?´Á("d›d?åÑ[`_!Š?À֍cúj?Ö~ÂůCœ?²Õö‡•?¦húP¥?'x"ꢛ?ã^Õ¦˜¹(?³âmaÇ	?ÈÌée'^š?¡!äYÆ?¯ÉÝ2R?˜<ž©¿O¸?çÐ'ÕS{u?¤?	,Þâ!MIXED4FGL J1748.3-2906?ïŒïícEJ¿ãW;P8&¸À8+Apã—êÀ9Äöæ{Ê|@­õ«"A;@ý%àdYF?¿Ÿ©¾×ý?ԉƒâM<Ÿ@E¿9fS?üóâہñ\?ŃÁ–ò,?â<AßÉSÆ¿áÿÊñ*z'¿åž¯ƒêY¿ë˜ÂÚÄ¿ïÿÙi"A'UNASNone?Ž0ò[êœ?œï
?Ï;?àÒüKPÇ?̪
wt£
?Ýk€
xÜ?̨>Yú>Â?±÷6±+¬b?µ*(\:t?ÕÖU"­"?Ãçdf?âÕî`47?Ä$"¼	R‡?´œøpÂõX?£t'š¯?Û†0"b?µ¡½‡·#?ßÄ;´4ç?µòR õ#?€µÃC}­|?hÕgC"Å?Áœz-²Yž?¡'2çT›?ëV
g{Óû?¢WïΏ$?"0ápßn?¦ßbàü­Ü?ãáÙ?掯?ÆH§¬µ]Î?ךÆuÝw?ÆÒ	Ö ;?'ó`Ë¡ó?š.‰;Ž²œ?ڍ܏£?Ȅls›®?â)8ö–Ÿ¿?ÈJk>ú«?©:}2
vê?œkÝ~(ƒ?Þùk͜«?º·!®•C
?ÝßECð´w?º[1XVr?c­ÕJo?T2/PÈ=ö?Æ'=í²‡?°
,åÍ`?êlH[A!ç?°5'õÿ{?MIXED4FGL J1748.4+1601¿ïÍÒèMd@4û3ÚøßzÀ:ÐðŽrôêÀ<K¡qÕ/r@Ɛ'ˆ(-@?']<9?ÒJ2žb×?Ù¦%ä@0ó@Àa"V!@Gœ¡¶Ê?émjf¦'G?ïý%?T©¦¿ç	¦ý…Qc¿äX,²²%¿ïþ\ý1§¿"É*gøUUNASNone?íò~ÒîÏ×?¡D@q–?"ÖϺOã?ŽŠõ'q¶†?¦lªó*
?›–<¸…&¢?ìÊÊ3je¤?¶I¹HRØ?«˜Ê}þc?°hæ<w?§»BýÿÀW?£ÖËK"ê8?ìb3™_?¤30p?–	?£aW{‡ò?•W›('-¬?³=·xÃ.j?ŸÄ'	H?ë"ÂP¶À‹?–˜Ò¿íü?°rñQ¸ð§?'B:íN¾?²æü'µ$?ŒÃ†ü(È?ê‹àðx×?µfN.]…?¯LÛïÒ?§ÒDýRT?»ØªóÖsa?±aà-–?è9¤*[/?Ä_d"®?ÁÉm@d
?ÀâŽ;R͔?º ,_"u?°îbN_Ñ¥?龞…Uƒ¯?¯DS¸gO?­|Ÿwyë?œô'õ¦Ú?Á¦^
§]}?¨Ýª;c"‹?åí&©."o?ª«ýîY™·?ÀžÅ—=7³?¦1…
dzP?ǬŸÄ¶?¤j7ùí`AGN4FGL J1749.0-2119?颢éñÃ@
0d‰Ø[À9…
a'ÏÀ:­y×\rÈ@»˜•±ƒ@<ó~}×?ÓÂìCŠ™L?ß¡2À¹o@ÛÐüv<?übJG¡Õ'¿à+"H×à¿âØÂ!y¿ëðÞ¤æ¿ëF®::Žq¿àÿñ½GÌ¿ïãtÿ†]}UNASNone?Û°µ+½Àb?Éc(Iå?·(«À™ªå?Â0îÊ½J?ޅä÷»ä?ÉÂòGä#?ØF« ¥?ÉPÜw Ü•?¾.?)FÜo?»{1¶?à6T ?Æ^%''?×÷>h¤ì?´{C É˧?Â9Ø¥kV?­2À²è>%?ÞëÕDÚ>i?µa½G9H£?Ã{Dˆ´Þ³?¡?Žôã?¹Ý·róÆ?ŸË}£a?çåwü:ù{?¦Ýð@ÝOX?ÕQI¦3¨E?ÅUSeúþ?¸Õ$	Ã-?´|Ûº#Èt?â<¶©—5?Ǚ;1Ñ«¦?Á@óЂö?¿˜Û?
?͍1ŸgíX?Çf÷'`¹v?äL±›1ãí?Ç^ûTö?ÏÌËÕÖá¤?°ûe²$?ĖJííŒi?±h†ð•@ÿ?âç:Oä}?¶OÆÅTf?¡åŒ12DN?‰'$àsÃ}?ÀÜÏë †?¬†Åß K?êªsB[³õ?¬Ì¬ ÅMvOTHER4FGL J1749.6-3143c?ïã\]pjïÀn²Ð¢DcÀ:ÔK3ÛÀ<j¦gv@`ÆyvŽ}@åF
¦L0?Ðô»¾²'Ê?ïr7Pþ@ù?R%g@=‰"~¿Öy>‡$L?ï5ÞUö¿¹_ò.+¿ÜB‡d
¿ïßëìd?ê:#aÔÜUNASNone2FGL J1749.7-3134c ?Ș¨¿¬?»É¦‰Ž?ѱ¸
;ì"?Á*O£›?á =ΨÖ4?Þ7'WIØ?»W(ǀ?¿g
v⛧?Û¾÷#˜X?Éu+ópG?Ýk>û›õÈ?Æßõ‹)`Ä?ԐN'ñE
?±žT; Ó?Ù!Ô¼°J?²ÍµhͶç?ÒN˜R
©?°Í6Þq6?Ö®EQ:R?²
I×èÉR?à)SÀ¶-?µFç.È¡a?Áÿä&Z²©?¤ C±ŠI?²Ö¾Ôkƅ?©Uæè1 A?Ô¤]žQöS?ÃÝ°,X?ãRùUۘ†?Ĕ-¥eæË?¥Å+'Õà/?°AÚŏ¿ò?ݝÉ£¹?υ!Òã'6?ߪCÄêš?ÎayHªi?ÇMe®°'?ªÚ¦àÇ.?à{i	{KG?µÛ›'h?Ób{±(h?²íKîý	'?½êp̛Ï?¨Q-šòþó?暜'Tž?¹o²Ú+w?Æ UWlÅÈ?²TAfJä_MIXED4FGL J1749.8-0303¿à"ˆˆODa@(q[Ývh<À9.¨mqóbÀ;\ý#¬­s@·"CñòK@FC´g?¸¥.ßL½Y?Ñv°@O%'@}"Ó8÷˜@2A~$ž?ﹺAn_¿á"¹"K‰¿æŠ"XŸÔ¿çu –
¿ïþ@½Šd¿ïç0ž-}UNASNone3FGL J1749.7-0305?ìÃ,z‡Z¨?°q~G®·?¬©ø=g4Z?¥.¥Gâ<­?§#@kS-?£íeKBÐ]?ٜŠãY'?ÈvŠuå4x?ÛäSÌ°È4?ÇñøúÁìc?Äþ7N±úö?¼' 'Æ2C?èzÛhq?±üHÍ?Ñ?½°›ö‡à?§ Í¶ôÌ°?Á	Ɨx?©0pôÕl"?Ý£³Ä>?¢•8l>÷?Íjúµ=d? Qÿ!ïÐ?Ó¦ÎáOÞ?Ÿvõª¼¦?ãýùã[Y˜?Ââ<W–Œ@?ÍNw^}±(?¿yçzÍü?¹¡èx?¶µ¸ÎD€?Ì6˜šÖ?ÄBiš(q?âdg0™XŠ?ÉÊ}`§?Ê7Ê çZ†?Á¯•ôjî?á²®Çì?¶^!Ö£í?Ë;ä²±»?±f¾*©"?ÐJ¨˜˜›J?²}·úió?Æ&;¼LT ?›aU¢¢@'?Ù>'gä|?­ª"LTv¸?Û®`qñ4?©sxÞé"ýMIXED4FGL J1750.0-3849?ï¿ÿª£4ÖÀz)³únÀ:FdÆSÀ<ø´²#Ô@ÝâF܈W@Xô›Gïƒ?ËJ}|­z¢?êÁLÁN¿V@ÍäKjb@šº†N8G?ìP¾´[<¿ÛÝÉtR¸4¿àÃ?O¡(¿ëúç\›Š¿ïþ'Ý¿áŠ¯ñʳUNASNone?»Én"æW?¶2õ9—?;?Ü©6Ä|
+?É$À9ýñ?Üdm´¼??Ç'ÿ9ËB?»—™SŽ¸?¸~Sp i?ßD yOÕ´?ÅR!_÷?ÙÕù0Øåà?ÄL¸8m–?Õ«™z©®)?²‡`&[^v?Ü9Wfc?³G۞½>?Ì6¬[àré?¬xÒ¼µYg?Î\ðŒÖ£Ì?¢õ¥ÕYÖ?â.¯ôWˆÜ?©Öëp½1˜?ÈèO¡Ë8Å?¢…=Kwé?¦¾¼Uë Ì?ªWٛ<[ü?ÜáS7"?ÇuOYÑÐ?à#j²j9É?Æ©?÷3J'?¥bRBˆ‰Ô?­9µ¬•b?âÉBãM?ÉÇ¥šó{?×Á0³mˆ?ÈÔè^<?Æ|Ò@ˆ?«§<äDµ?âDØ_…ª,?´Ë0'2â?Ð8H@‹‹d?°Îè?°
Âv·¶H?'¨âé—ÿS?æµ @Å˄?°Ðß©cà&?Í$¿Õ(Í?®Ô`šžMIXED4FGL J1750.0-3347¿Î׀7¦hÀ
™ÔttFÀ9Åét£@À;HöHÇ/@\ÜÇÁ @}N?(3ü?Ëøg…JW<?ÑUA8Úg@†&oÖQ±@¿"²²oS?ïüë¾TŽù¿è–µ¹ŠÑ¿É!"ßù$o¿åÞjNRsj¿é±y?%3¿ä¢W
--UNASNone	?ÛÊ)ƒJçt?ÀåSýê7R?ˆk8—=?–€:/Î::?á¹?1¡Á9?Àø0)0¦?áóbhF?¿vÚ¹?'ß3!'–$?ë™ÐýÝ1?ÚûØü92?ÂCÞ.҃ù?äMºk~ܲ?±®A2²Á?£ü¸=lÉ·?'…buæÃ?Ôäô!‹§$?±EÖ<?á!ҙ{¢Ê?£ú5Ê>‰?¡rßLÜF?z½CŒÛ'Õ?ێ0±+d?£³~Ë;?ÂOŽÏw]@?²Ý6»ù¡ß?•E¸íՃ?|~¨<û?êÁóú"ô?³öXk¹Òî?ЬÖ<¸3?ÁÌü–Ð"?š}Ú; ?ŸHÛ⧆?æÕ¨âü}Ù?ÁÞÑWÝâ?Ó~šÈ¡LŸ?²Þ'NÕ!Æ?±R16j?—÷)dÚÙ?äÈUCÔ@?³Stah?ÐNö¢‰,?¤»[°0Þ?¨y×EAj¾?ŒÏ•¼Û·"?æQYúo®?¥·¼†áMIXED4FGL J1750.4-1721¿ÞGž`cÿ@	$kðÀ:òÕuûÀ;¶၏¸@¤X[¶µ@ 6^`Þg?ÉϚ‡€<{?×ý¾¼éªÔ@»A®@ñ@…šPΤ"?îðÉ@Ñ+¿ãÁ9»ãp}¿â=d_%)…¿è_‹*ì¿ïÿÿ" 5•?ïÿû-2h2UNASNone?Õtë9tk?Â+¡úQÝ?Àc¶/Òð?¸ãá©?áXØWQ?Ť‹1™L?àð
ÿãO›?ÅÖ봙z?·3õÏG?°¶‹>xeá?ØRìŒۇ?Â*EC«ü?ßjLFvÿ2?²:£×ðs?ŽOA9c×?¦
QÍ':¬?×NŒÙn#?±>ř™òï?áÐ6Ð1íI?©Ö8žfŽÔ?¼@˜}?—\¹¶¼âk?ÕOl`¿?§"œ5¡?ÌN¿«§
?¼=Ø2—?ÆbïÑ/?ÀUkÙ3?ãGp[Õ
U?Ħµ…w<'?Ë¿›¥§2Î?´!G"?Æþ^ˆT*'?Áï:9Pk?ãPt(¬?Åk"ü\:?Ô
ì}tÓ?°m§Â4?Ê@!Y ®?®°®éIö'?ÞÒҒUúÖ?³Ÿ©¦f?Ëï$ ×Í?¥¸:¬iÎý?ÈO¿<¼?«Q@öÜb?ã+TqhÅ^?¯#"9ûpÇMIXED4FGL J1750.6-1906¿íkcϙl@Q€Ø´À9lm½r¼¶À;	:×lc@"!"9Å@þ7"«üs?É·¸=žœ
?ÌϞxÑx@}£!ØG?÷ô›ï	?ì4јäh¿ä×ø¿Äс¿é8Ï>ìúÀ¿ã»?Ï¿ì^ý¼Xá¿ïý‡ŸñøUUNASNone?Ñ[h×Á?Å5ƒ­Ò"@?»¾r	:nï?Àær?ãÚ£
lÑ¡?Çuf—r?ѺÅÚ{rM?Àó×
ÿƒ?È8bÁ…	Ù?¾ÛOÐ?á"bac?ÁVš÷ÄÎ?ÜbvM X?´)È0/óŽ?¾P¾gQ?¦\0dP?Ü	Z‰Å¢?³g(2'?¿'ô•ž*?"kTcŽØ'?ȳŠ˜Â&? ×¢9ŒyÝ?åî<Š¹›±?£0Ú~ò?Á¯úóÀpb?´<ºÐ³Ó?À6;ªê5?¹|¶*ÿ?ç†r€%)Z?¿R›‹ë?¶=¬÷A?³¥üDä;?ÒKÙlS¡?ÆögZ­³?ä¿t8zà?Å]âzDO÷?Ðwð÷úM?¯•Z¸»Ñ[?ÁÙ
¼šê@?©§Lž^èR?ãMÄÜé?³FÖOüÍ?Ÿß'2Ôüb?ü_b:?ÍځWû¶ç?«¾°±7?çŠc˜x(Ó?ªýcµµm°MIXED4FGL J1750.8-4405¿ÓCè*SïÀ!Jæ…Ûv´À:gþÓ°ÝÀ;àZ›W	@öä¡TÎä@Ò	Å{Ÿ´?Ðúk _pÿ?Ú?B5.µö@ž$»¡+^?ú¸`ygu¿Ø-³Âd¾ñ?ïÏ¡ýÁ6¿ÑµA*l»¿ä;ñb®K¿ïÿà?Æ>"?ïúñm–UNASNone?àKU9©€(?Âée+—¢?´¥na
±?¬|чL?Ú?ùô¼ï¤?–Q
—Jè?â)¯‹žY?ȱÞð÷á?«x5…va?¨ÕÒЊ%?Ø>ç9"'B?ÆÊÑ6¶Aè?ãY‹àQ§?±œiÛN?¼§µ%¼'8?¤h·G¬d?Ò"úõîÈå?¯»b¾6?åÖó|!?§¥àžE?¶"³œcÉ4?"}7¾QA¹?Íe7"'7a?¤´nÿ^'Ó?ÓbXM&¬ñ?À¶Jd–ò?ÆcY±Í?º3¿l‰bŒ?àµóƒ6B?îÂÅ%Ó=?Õ=ºlM?Êq³p9ì?¸?‰
ˆÍ¢?¸†sãĹm?âY1¨ª¿Ã?ÌÕ²'ôª{?Û_µœqD?±ñ0?Ÿ
ˆ?ÂúöQÖa?¨¦†,£xË?Û#@é̄J?³ŽÑÝv	?Ú¥ýi''ä?°5a²ÈK?ÁЬý¶?¥Ên£¡°>?ÜqôÀlþA?±Íöè[ûMIXED4FGL J1750.8-1246¿Ù2"%°‹@å$9›,AÀ:€T–ZIøÀ;©Äÿxñƒ@2ް@º<÷T?ÖVԍ‹n^?ã<¥7\ @"ª^ã»&?÷y¿¹†?ïÿÁ¡u†¿à}i[
¿Ø|1©Æ7‡¿å@p"|ח¿ïì[rí]f¿ïäu_þmYUNASNone?—vÈå?¼¯u½¶M?—;_ןòK?—8×s**\?ê G{>º¦?¿<ýXÓ"?ÕOý?C?ÇößBκ@?ÈB…Ý5`ñ?Á®w…?ގÀJD?ÁÝ˞_¸3?ގüwŠP&?±ê´Æ#?À¤jo¬Øˆ?¥"Füæ0?ÙÎOŒbØ?±r·ZœD?ÌÈÐLøÅé?žؙ{êò?Ë_ôœÊ{?£ƒdA%»?áõÎŏ/¢?©+>®U
?¶ÖglîZ?³<w€†?™"_Ó+4?›Ðh9"˜ò?ìX˜ÿޔ?µÝ¬Ã?¾¿ÉŒ¯?¼à¬þ{Eœ?Ñô⦏?È¡©?vYñ?ã-ûÝ Hy?Æÿ2ÇõÅ?ÕR{'h¤¯?²Bþ)׍ó?Æá=ÒÉf?¬MOÌÃ}ô?ß<åï2¨I?²óõˆªIo?´=GµÖy?'šBz½¥+?˓jŽ?°("IU}?擐¥¼?±-"
TùMIXED4FGL J1750.9-3301?ß|0®"ÉdÀ¡f>ù:À9º:NÀ;9=e¼{@Æ<幃@–õw/?Éú»¡ w?ƹ«R5Ø?þ%½ÿªo«@v:2€Û³¿ë<":µ´?ïñ@x@.¿æo;At"|¿äf†a®pÁ¿è›
²ái¿ä5M>ÍPUNASNone?ãD»#Š§?ÁƒŽðží?~±Ùפ?~>î?Ùw'ñ2?ÁŽ$E"™'?ã%®—ÏâM?"†çݖÁ?ŽŽkƒ_?š«¨¿ñ*?ØĖ`1̉?Áó´ÏøGÇ?åÔ¥âäL?°Y:
SE@? ê¯¡?y€"
ì´?ÒV6ä©Éy?¯RÞBlÁ\?åÜí£©_? +¬â9o?£Î«¤R?€ß{N¥ó?Óvp°ÓX=?žÃصÍҒ?Ó!©üpÜë?¿>´¹cA?"¬Ÿ†ý?"בüá?åÉÆÒ%k?À
"Fö?Ó{-ƒõ?Ë©eƒVP?š˜Àl{?¤$¬Z,ˆ?åm£m>-?ÃzFºp÷?ÕêO‰Ö+?²Y"½ÇX?°Ù•ÉZ›e?œMn¾f¼ÿ?â壟(^?²y™Å1¤?ْràêˆl?¨¦Æ¼ˆ,?°œ+˜›S?""öÎ|E
?á#E
\`?¨ÝARõ_,MIXED4FGL J1750.9-2655¿åý|ô?"¤ßʚ1À9)LøW>À:ªo ¡Ë—@Ýèuõ¥‰?ÿe©Oð?Ϧ-ü'6?áÅ»ámÛ@ÛxFbºà?üAmwþ?ïþµ}$îÍ?è­½¨l›4¿Öàæ?³¢¿ìzD5ë¿è¥Ùä"s¿î|¯þàÆ)UNASNone
?¢äªð÷&ý?¦=rL.Ê?ÂÄ·ß½±?£ûrW¯k?îKŸ+1£?¯!›õÙ$?Æ¡N	ßc?ÄÆr6£f?ÀWðö»?¼n9ïdý?æA°uÂéŽ?Å×+¢'ˆü?ÎoA4s»?¯¡hªjK?¿8^sÜN?¦ÖÒRPbw?äH§0'‡?²«—ß4w?¸M5([ð?© ¿%4æé?´ü%ÏÏ3û?§/|X5ä"?êVÔ ß;Ã?·?Ý&~r`?–Wï
Yÿ?"St":P?ŒŒ#¤Ž¯? Ì7"¤"ò?îÛ;Â	6?¤¿Ÿ¢ùé?®8¥=/Ä?±Çßåôµ ?ÀØ〲1?Áå9d>‡¿?éæpsÝs?Ãr/@õ5?Ås<Á/p?©N‹=P?¾S1¢±¾?¦¬±±4ã.?æцiå,?°Q® ùÆ?ª8Â~À$s?¡'¯½àZO?²ÃÝ>›?¯߃~gI?ì|5@æ?·ÜÄæOTHER4FGL J1751.1-3455¿ì­ó·X'‰ÀUiR‹¾À9ø'õ:ª À;i²KAFò@_fPÁäf@ÿ#a.?Ê´®ÈÕÇG?¶)vpõ‹ˆ?ñÛCˆ×?÷WdZÈx?ïŒ$Ñp |¿ÞâšÎÍÙ¿ì{´ÚgÀ¿ÔBe"oä¿ê±ó˜°Ý¿ðUNASNone?ÉÁ"Uuäo?À	Éb4'¥?túö¸Ñë·?pŒö¸'ø?ée¨ýK?À8É	É­^?â	VÜr?´¡rVË?"ˆ©Q?55…·©>?Úî´ÉJâ&?Â@Ôúv[Ú?áÁu¢ˆDv?±•HN%çk?ªI[Wƒcf?™Ùê21'8?Ù3éOÿ
¦?±"œ5ãä,?áÚQîñK?­Sðqï?§"5)8¥¼?†Øó"G.?ÙZÕ}dH™?­uàãÍGÜ?¸$jÇJâ?²pÝཽ?€vO˘çç?}¯­ü(å?칙g«Æÿ?³7g÷?ÐR(±¤þ'?Á¡LF檀?˜Ä/Êfù±?¡ØúÓQh?çÊ)H<Ÿ?ÁÌM…Õü?Öf']Ï­Â?°6žc*?´öÍ£Ô|?¢­cÿÑ(?â-Ý®qm?±8-Iãn'?ÒÃeüšV?°5Qà¤Ca?³Oiù®ã?›Š3nC3ï?ä4_Âw":?³r߅
MIXED4FGL J1751.1+0109¿ÑÏ}T?"@+ÙØ@žUÁÀ:E,YûÀ;°"L*zþ@ë"Ò/bC@œ'W…øÓ?Ԁr¡]2`?è*±^Ý0@Yàâi?ùøYMN<y¿åÚâ9E›ì¿Ý¿‹0JJ§¿èK"¾h…û¿ìœ.¿†S¿ÞÞõöÕ_¿ïó"כ\èUNASNone?ᣦnïþ?É
>=8«Ô?›î݇žß?"ƒ¡eVK?ÚùÅJÄÁ³?ÉPëf&5Û?敷̬ãÆ?Ë$À(ς?śëîÑ"?ď›~v'¥?À
4Þ{mV?¼»ç.DXl?ä¸Y3«‡?²'!$?¸ºï†‰g?£Áx˜´?Џ'I?°Œ&ÿœ?ÝTåF㋣?®Ob]«r?Æ\ïB >—?©ØQy"—?×|£U?©S>€AÃ?ß#ô1Ö?Énœ°Ç«?¡ÐƎf­?› íb"ó?Þ¡òx*+?ɖDB?Ù4·‡–6ä?Ðæaä ¦i?ÚAoÙN2?Ñ÷æð©:?ɎF·R?Â0øâ:®c?àKå$m®À?²‹Råó<ã?ÁÕîÐhôÇ?§¼f­qp?Ö}>Nð(?²<æCÏ	S?ÄkiƒYï¾?¦ÚhÅ%"?Ññ¬ã×´?ºê°Á#?áìO›Á–?·Jºq' MIXED4FGL J1752.0+3606?àóm@:î®ÀrKwÀ;nƒÚ³ìÀ<ÎI2xù@ ICF¦­~?þâ¿b€þ˜?ÐÂHyìU(?Â+ÍxÄ6ü?ó¨(Ãm¨z@»Ã>-¸?ېR.9#? El¿ÐZakTã¿È(aP¿íXØãÀ¯?À[˜·§wUNASNone?ï¸Û"rh?uÔÃӊDR?cˆqlî…?[²uUÄ?z*˜dMM?qA툩g?ïÍxJáÇþ?u¿Ì¥´×?Q
c¼Ùà?YŒäÓ?uA€ùC´?pqƒÁD?ïl6p:·?áZ"x#?wöÈ΂Zì?x0©'@x?™Æüø:n?ŒOr'?ï}4ÌÃñ?lôÙ6…€?t]é)£·0?YŽ×sÄÈÇ?†ƒØHHFª?gZªM£?ïqÈ7øÐó?"'UWÀô6?t&£¸s?k4Ý,Ãcâ?‰€^®7ë'?€§Ù'˜<?ïp‡¦kÓÒ?v1ûô¯?c"sŽd֝?uE²Pj?Žù9†AI¸?‰rúÞ)­?î¬АÒ?›^Ò
øgå?€ƒS¡ÝžÎ?ÍïH'?ªifãô8?™rË^¯Ö?î¹³È9?‡nyU7‡.?"Ý!Ùú?v¾U?ž[¨ûmf?ƒ§Í5"ºÑAGN4FGL J1752.3-2914?ìR×ãk¿öž²r®sEÀ93âÏòÀ:N:†
˛@ÊØ"ì>,@zªÁ	J,?Ïfކ]§¦?×Jë I÷p@	wß 'á?þZ2H|›‡?ê,n¾#¼ž?ѺÔýÐ
¿åøÙÀ¦"ê¿ê7ÀÌ
Š,¿é¾u†"Ú¿ÆÌÉ\Tê"UNASNone?¼@íů'?³·ÑÌ$¬?Pô'£+?Œv'–`£0?ëõt}Í­•?´¨šÐ8?ÐõGZ1¤¾?Å ŸÌ}`m?°Ûì?Õ#?«\7ñ*q?åiÞËnM?é‡xYØä?ź`½É¾i?ªYÔyíÁ_?³–6ùì^›?ž­6nÇ¡?è ñkr?­ìóÜü²Ó?±×ftLZ?ãÏâo»?¸}Í췗¿?"Ô›mär?êÎkUc‰½?œ›ÆDhÜ?¢ø7€W?œª¶]{"?ŽPX̹›[?Œþ9eÙ!?îW6©pm?¢Íðúƒ³6?´'^d-?²G]€ Œ?µã,¡Óâ±?²Äe{?ê¾®«=tÄ?·Ã.Ýqß?¸èVQW?ŸIsIJb)?³Í/ޔöG?Ÿá²Ðî*?ê"gç"—?¨a$×&¢>?ìñ׸É?y'\
ÌÈ?¼•üÒµ*U? I®a=!?ëåØ݄Þ?¡ð[û±ðOTHER4FGL J1752.3-3139?îË^"'À ]ˆ¿À9¡w·ÒjÀ;HóŽØu@DPó7š¡@õö&bjX?Îê—Ä'P?ÐY0ó½Ò^@uH#…@F?ðèҁӿìTS^¡Ëí?ïÜùjºˆý¿è–"ì"¿æ•BA˜ü'¿é7zàÆÔ»¿ÞR†à"d©UNASNone?օ%T‰€X?ljÁTž'Ó?§£ÝxK·?¢®	q¦ˆ?ãC/~Œ'¸?ÈaÒV
?ÓuTé™ê«?ijŠÀ|¡*?¶§!üÛÜ?°m0æïç?ãu`§-Ÿ?Âù=ßð§.?Õáas&W?³ÛŽsý?¶`'_˜j?¢Ç¶Ù¨?â¦}ˆ87?³LOb3"æ?Éíhmý‰ƒ? €ÙYM?Ɛß÷!	:?¡þˈ»63?ãàmæ¸[Q?§Sò…?ɦŠ^ÏTx?»3–°['?±@§Ì‹'?«J2R]{ù?çnHnÈyp?À˜UgÌ©"?º"‹€¯Æ_?·IÎè÷Hù?¿vR >ù?»py÷?è¾Ä;XƖ?À¿LÖSµ?Ä\ùÞ±Y\?§Á½cÉ	;?»®?æA_h?¥õJ.ø;?çrù‹‹}¼?¯½‰z
Ã?³›&I\­?•xÎfø?É­8̔?¬­ ;ã»?çDïî1mÙ?®]o4OÅOTHER4FGL J1752.7-3040?Ùg#~ùôèÀÅ«ÀãŠ~À9¶4EêPÀ;?ª9ú͑@؂Žs@–üõ‰"?Íi#šŽâ?âAº°j–@¥ò`L–?÷IŸsxGº?ï!FÁÛW)¿×Ï?"ª¤Ú¿ÞïåÿÏ®¿é¦2Ï`%¿ê€™'ódç¿ïö×B®\UNASNone?®¤Z4å?¢Õ2wё»?©ìˆdI?£µ¬S=fS?ìvñЁ&?®œŸæî>À?Æý-2KÝ?Á:tOÞ¿?ÂÁÛP·í1?¹poýšk?å=ÞÄ]?Àep"Š£?̓ÅöÝ?«£K?À"ãzÊ\Á?¤e2òŒ1?ä}ÕÞâ™?°õ˜Ó üd?·cÿ†öc?gú¤Ç+??Òo›Kþå?¢}æH¡Ò?äå²và1?¤Îêþùá&?—:[_fÝ?‰Ì¦³É˯?­RÀ9"
?¥àêçŪ?íq!4¥q?¨€Óã¸
Ý?ªácÚ??«À°½U>)?Å_±
ÏfÛ?Àµ'q×Þ¤?èú§¥?À©Âï/?¹÷v¯ìŽ? 
øyË^h?¼ƒH'Ƚ?¦³ÇÍq}ë?é0¨%<iW?¬äªôfÂø?›BjÄÖŽ?{l
yÇ¿?Ó­˜v{T?¬®Áæ=+ó?åšÝâɹ?­†:|8OTHER4FGL J1752.8-4449?ûÞàBóÀ"¡ÿ´€¥­À:9·	ìèÌÀ;éBí»YÞ@—M;@3ÁÎl	?Ç·&'?Ù_™ãÁZÿ@çń/_@KÐÈ:?íÚò)}§Ì?ì,â·Ý!¿Ù( ú"¿ã	Áv,'¿ëÜ>"Ë¿ïû¬áxUNASNone?ÂÑÝ"/Ê?³GJè²r?Ò»"ͬ¾?¿wàùL?âJ+&
I®?Àã¦tÄ?Öâ_`´^?ÇM/·í[|?ÇUB@†?À9kU'h"?ݗõþR"?Æ_ɏç¥Q?ݱä>-?³º\¦>ۗ?Í!…QÊ3Q?®¸6cz‰ð?Ô_‹qÉØ?°³àÉA½?ߞeÎ÷ä?£'=TŸ>Ÿ?Íæ:Y~]?¢fÿL'«(?ÑnŒÉHî? Ç˜æƒf®?²£ßõÞÃ?¤ßäžÓÿÂ?ÓNj΢\X?ÁÔièì?äN™ÉÌ?ÁUùV'?ÉzÇ7rÄ)?±ÃJHÆ?ÑcÄ
i'¿?Ǐ$jî`p?àïl+n»?ÊÒbDæz?ÒIý^(îû?±eùšeem?Òø8-˜ê?¶ñ@.K?Ú½ûi©x?µ¥P5â
?Ï¡H´°v?¤ÕTkù3™?ÕʽàÃ@?°£"=ß+?ÚdÅ3Œ†?­Œ~y¾ÄMIXED4FGL J1753.8-2538¿é÷'HD‡?À?^¥&ë|À7´ªÄdHÀ:L$BÕg¦@þ¿e @ìÊì"?®c_/n
?Ô/ÆÂÃÖ@#š {5?øƤfý5?áÔS»d?Ù0W¶ :ž¿Ò•ŸäâBU¿â€Õ}uv¥¿ék¡~•\H¿ì¡¶hÝ9,UNASNone?i¡Ôb+?e°¡À©Ö?åŸ0Õ¾k"?ÇÕÌuu3?ԏaÁu?ÇÏ/æv?|DçOTÝð?ƒñŒõ ?ç]X-Ç2?½K Ê1ßC?ÐÔ<B>"?½5TåNg±?¤õ=¾®OT?šU÷Í9UÍ?åяª,?µ)qô/C?Ó)µ(žã8?´©ßëk&?j."K3?Qav"€7e?ܗX¤åZÁ?°s`@繩?áš$ë(5?°«ù1?nð:g"bÍ?ehçošR‹?åŸ$`1™?Äb+ìökŠ?ԄAs'Ê?ÄG¶pa^?qè¿÷›:U?zhHŒ3q?çáEºÊ@Ö?Ä4TE|Œ?Ï룈S?ÄNԛŐ?¡j()ú+?—ö‡
ú!?åôrn:"ï?¶¢ÇcØ÷»?ÑöÞØñ|?µ‰!;šJ?L_±lÝR?8™ŒÍÂ÷?Þäg7
?¹Èð_©'?àív¬A?¹!Ÿ¦O¿ÄMIXED4FGL J1753.9+2443?î'Gœ\þš@7û¨'j©À:2@h¥ÛÇÀ<[š'Í¥:@҉¹ý'=@ÅΞ^$y?Á"K©¡¤€?¶@+"-t?õbØ<l˜@
ÒÐ]t$?í˜ø‰éù-¿ç$‰¿ß~Q€ž¡¿â7 €=¨¿áXK»À5¿ïÿ¬ÞoâfUNASNone?ïñêә?WÈç¼D›?5!¨]Nw'?#g°7z{?Vãl:T©i?V€ÄtÝLJ?ïåP²}žÅ?lIŒ…X?=–Of39?I¦">žå?füŠC¼?g‡ø5Ÿá?ïÁ$S'š5?k5žEnÖ?T'cùÍ×|?T^Ÿ·±­Æ?zM=P
£?h™8e?&‰?ïÐF4ÓØk?RYãv»S?N›ãW-]?,ëèÎ~~?t	i2Žª?Q:ŽÞ3a?ïé|‰$Ò?_ÃSV09·?A¸ü]ûˆ?3&¨!éŽ?b7ÐËçÏ?]ÂöDufé?ï¯)1b߯?'IŠºä?Qø(Ðä?^0¦]Ƴo?'"'ÑÉ?€MMÆ<$?ï"ÂÕۜÒ?wH="õ?axqxä¨l?d箘ëÑ?†q.¹w'?sfÈ?ï'jJn¸?oÝIÌn¯h?aæSn*—¼?GÎ
Ê>žÑ?Šë؎sŒ?nkŒȂAGN4FGL J1754.1-4333¿ì'Ö_À!ϪŠ'¥aÀ:åªô4ð£À<Taä ¦i@!®ˆ Ø?áÔ"°Õ?Ú衾V?èçԐ­?þHż7SS@ª¥¼'—ó?ïù
ãˆÐô¿è¤±ÅàI¿î½_œr½?Ë®¿Æ~ÿå?Á4Æ[C¿í¥qß@lØUNASNone?â¦ÿBë·ô?ÊÀzÄ»?_Vʸ…£?{)Hª:?Ú4"Ζ??Êæp˜œ?çNÞ¸Â?ÉÐN®Üg?r¨QÍò?ƒªmW4?Ñïý?Ét"úßbY?ëmøB*·?¨:ŽkD?Š×ÿröÉt?†á"Jð¾?ÀšŸ«"ûO?§W{ Œq?íubÒª~¼? ¬Ò?PÃ?C=;ؓº?EŠ\"Ï(æ?´.nôY¢–? ¬˜pkü<?Û̶jU?ËYñã݊Š?Ž½ŽŠTª?Œ©ª,²¸?ᡉÿŒr?˃!ׄûl?àrÆç'?ͱÇûN6ç?vÊ×ÝH¯?rŠmü?ÞÀÊb0Ä?ÍJi…ª¤Y?çs!HW»?±:àY5j?•#i%X`1?*³€øf?ϏJUŽ§Î?°·wV÷Ô%?êg!š?¸£¥>XúD?L´å™Z+0?Wâ8[ž†È?ÆFÇ"‹k?¸¤\èZñMIXED4FGL J1754.3-4443¿¬ÔìQ³À"ûR†µ'GÀ:x.åƙÀ;Ý Y§;@NµÖ\@Ðä¤Yæü?È;>"õó?×Wôž"}@‹š°@2+5㼨?ïý˜F³B¸¿àžÜd…¿áø#'¬?¿ç²ñYt¿ï='á>sÙ¿ÕyF<û3UNASNone2FGL J1753.8-4446?ÃGYI·ü?¹3s‹I?º4w·?²çΚ}%?ççšÎui?À`=ø‰:?ÝÕv!¢ðŽ?É0­ˆÛ0?¹"l3œôõ?·H6v‹W?ÛÅnёO?Ç5üíð?ڐ'ÆoD?²62Ql÷S?½¦Íãçà=?¢èHw?ÞºÀ–ï¬?²¸xP?Úònk‡Q\? ÓaZp¶b?ÅàY@&û[?–Ê2MLg?Údôe0ö? ¥¼®ð¹~?¶ÄÏ5.v?°Tˆ­ãþm?¼òþËÞ¡r?µ58‹«¨?é çŒtJ³?»Áµuð>?ÌÌ"Ç?Äì0β?ÉA;ùD=á?Å*[ÚW‹?â|'t/'?ʘèn¾Ï‰?ϙ]z•®?­ð«IU?‰m$y9°?¨s¿uŽ\?ãwMX<Eð?±¼?0É]?Âjä©?–­/—€i?е§Zó?¦T"Å ?ã
÷«ÙÉF?¦0È#·MIXED4FGL J1754.3-2915?è~­|ûSH¿üÙ`sÞ.À:<Ñ®³ÝÀ;Ï!CF¦­@V'ýž%ð@•§Yu½?ֆm'dsÈ?ïâp"&ñ[@c§@KIª?ýž€ÌC:?í«j¿îþ@5û?çÕk׿o¿ê¥_Ù.…¿íÛÇ4ÝW¿éñ\~†ÝUNASNone?Ârìuxl?¹¹›ÇAÈ?Ç+ì`¢?¼/㮡ϯ?å®h-eé¿?÷ðÎ+>?»¸kä!?À¡¦>©Å?Îc}=msÌ?ÆYz¡ÿ?å®™
¶*?Ä·x@Bà?Ô}óâ$Å?±=½îÁò?Ì;y"6—'?­'$çRût?ÝdP<§?²"Tó¥¾;?²!òæÌY3?™õWúJ±?㦠÷Z?¼¨=vX þ?Ô*AXK+ß?ºƒ«±E?­¸'ßH?«W=*=W?ÄÐóD}*?»Í›Ii?éAðÌl'?À€QiT,}?¤i&Ýñ?¬Ör±Ü5?Î7'cœ ?ÉdŒÉžçY?ç+‰¥Þ?ÇÔ?gžõ¤?Év'ÐÉþß?«Š@%ÙH?Ñ@‰m&žû?³î&Ÿu'?á•:0Ë?µÕÖh…d(?UaV=@¬?'íþvñ*?ä«
j÷_?Ãq¾d»Q¶?Õ¤Ùsƙ?Ãq1_bUMIXED4FGL J1754.3-3236?îMK°¶hÀðƒB?@À:ðéÇ´À;}ƒvA¥½@þŽøœ@·†ªØ?Óý31…´
?çÜÄA
Š@~}ÖÅt@7§î&!?í Ɋ"-?ìT4ÀQn¿ä3¬Õ¶€Z¿îF—> Y¿íõ~†mÿïÉ$i¢UNASNone?º­x1âÉ?µ©E˜IŒ?À¸ü_?¹h1ÄR'º?è|öøoh?ÁèA̗ây?ÄQüæ´Ä1?Ày_
ô'?Òïû/hñ?ÅA";á®?ásƒ:»{?úö÷÷&?Ñô˜áÁY/?¯úСZ½˜?Å+<Žü‡¥?©¯ø]Ç?áºäké¡Þ?²uv®'ëÊ?ÁA14ü?˜)la²_?àÝ?š/ý°?±8»V
×?Õ¶`2ßj"?­K"}‹ú?°¬Æ·sš?ª¹ öÚ7P?Â#ÆêÇ?ºñ"§Mr‹?éd}¾Ùû?À6ßr
Zÿ?°—g1´Ð?³}5KA?Ö¦Öµü??Ë.ÉÆKî?â¨Á¸ºÇ?Ê'ÀfHE?Âmð0\È?¥-È×s­?Ç.+eÎ)Þ?°Í€¤?å™ë	ζ?´ƒ—–?¦tŠ5`z?‰õ¤a'¤Ú?áåÒ:Ü5?¹íöé	:?ÙeÊCIo¤?¸|ø²°v=MIXED4FGL J1754.6-2933?ìZ\áh¡eÀœ˜†À9<;¨LºÄÀ:ѕç]qË@ƒÅ[¿Cw@á';×F£?ÇFŠ¡Y,?Ý°å:¬Ï@¬$=Ìê)@Õú¿ïàk]¾L?ïÚ¶š[`y¿à4v)R	¿æÉúŠu9h¿ìÏÝ=]X¡¿ïÿC*!<UNASNone2FGL J1754.1-2930?¥2Vw,ž?oÓ«öj?ѕi&gÑ?ăKì"?åä'&½?ĺ·
?P?͂ê
k?…)é,ü?ÆChÕ¬o_?¼~ÊîË	?ãkI"áŽ?ÃLÂp¨^®?È46©ê?«[+N&By?Ðé‹ÊNe?±6ÀŸÄ‹H?á~,™n¯?²Í†¬¾Ç?Ìzôe˔q?£µ:`®S€?ÅTkKA`·?ž€6ÔÏæã?ãŒ(F3?¨ìMîæÌ)?¤¦p`?šë™¸ð™R?ÐcS—+Ö?ÂhJ%Vëc?æƒõג?Ý'®?¸Ðë÷R?¹Üw&â?Î7
â‡Ž?ÅVÓi|£ó?åo	ª#?dž†ä­Œ?¸Üj?¡£ä¯‰ž?Ó9"?¶IW–º£?ãsoZD³Ó?¶´µ"zí÷?¶Uo‡Z#x?˜ºáY?Ê×ÚXíØ?­b'Xl?æ[Š•DË?±[Y"õ.¼OTHER4FGL J1754.8-3200?ï¼î…À
*s±éÀ:€aº/;À<AÎm¶¼À@zS¶xM@XÜ}Cø}?Ò	}!"Î~?ïö@líüÈ=@4¿ÆÔæ!?í+ž{ÝÇ¿Ô5edd¯?Úø¦¥×¿ß½Á+®Ús¿ïýÝ¡s²?î¢ÊšÃeEUNASNone?Ñé×Ae?Ãóڀ&õ?È/'Á8?ºE<µ'ôd?ásƓD7_?Ŭê?Š–?Îòd?ŗ/ÅH&¾?ÈÇTaoöL?ÃÖÏܪC?âL)ë)h?Æ*smáZ?ß9D$>û?³Íâa®z?АÐïé~×?°"‹/'x?Ð5êëúB/?¯Ç6ü9£š?àz,æVÐ`?²ºô'ð?Ó&á|mu?³ŸöâÂNç?Èþ¡†"?©q-ƒŠ¨T?Å®ASSÜm?»ÕdȒ½?ÆH&¡÷®o?¼ÃÃBà?åf­I?Ãôó8µH?¶Ú3zœL~?»%´£ó?Íç[ü!›~?ɐvè9?åªâ'Û	Q?ÉÁÜrÿs?ÒÐ*éýN?²›X}Èí??×aqMäÔ?¶šõ'^"?Ö#s¤´Í?²è¯›—?Ê`¦?ç˜ø?±ó<-ë½?ßê‰:¾?À…Y;'?ÓÆÂVÒÆ?¹¡âÏ¿	MIXED4FGL J1755.3-3937?ïð#®ÛËÀ žý†¨üÀ:Y‰SÑ8lÀ;5^†ž@'êF/dG@bû…Fü>?ÚâLÒ?Þ]C½oÑ@
S½Ö.u@ÚÊö†?ÖªtÞ#aY¿Ð4à²\Þþ¿æ<˘fÙ¿æÎG P¿í9Ž—¿ïû
¢ò)UNASNone?Ú>;9'ò?čãýYÌ>?ª€_ß)>ê?¨…$×?á8Üe7¿?ÅÙC}®,?âÔIÐ|Q?Ưð›ç…=?©iñ²í?§UŽ†MÞñ?×*JAþ¹??Å	¨Œóæ9?àjß(¼Y?³KÂ൘ñ?·è˜^ŸâM? ©'õ‹hò?Ù1Â*Žº?²Ÿ©A«?âx[†c‡?¤Ûž<?º#±yÎçÉ?–±=ÐÝH?Õ<"ê?¤+mËmMÍ?Æ7ôT$?·}±ê²á ?¸>릖R?¯¬0–"e?çj%vؔ?¾ê³<­ÛE?Ô|?¶Ï4†?ÈÑƗ堔?¿¢\z™$?¾˜54ó°?á͔•ECx?Êi•@ª¦C?Ó§…"ÂP?±&
d^Ó?¿û–cÚ?¥ëˆS
y?â,ýðÂ[–?³"Vª—ÔÚ?ОtKù ?§µ!ª1²Ï?ÂՓêFôö?¯2eðÚ$"?âû`ßqr½?±sšÏ¡(ßMIXED4FGL J1755.5-3734¿Èi8}ÊÜÀÂu%F
¦À:3qxéêÀ;´Ç%Ãß@àÃEJ7@¹}£~?Æda¾áҘ?´¥sl‰@0?ðËoÕzñ8@å½ïD¿í
Û¢R¦?ïâN>Qtg¿ëô…þ²"'¿ÙÕp_c'Ì¿àÍ]ìDaY¿å3TÁ"tŸUNASNone?â"m>`¨?Åb]5mÓ¡?uì><Ç?låµÍg?څat L!?ÅhÄ3¡?éÇ&"\(þ?»%hý­?jz=@¤Ì-?p(v™tè®?Èy~'M2õ?ºÆ{"z?æIÄ»¹Þ?²:üKÀ{?ž¾‹1x¨?'o~Ïù.?сõ}ðñš?±;9pá?í)ùa'{¤?Œ»èžD.?ƒŸ*¡˜p?e×Æd3?´<O"Ss?Šþ5ɒ:?ÜHcü©´D?ÅÌt§
µ?‹ r=?ƒÙ¯æbw%?ámL9œë?Å=)H?áëÃm' ®?Åèxüãb]?xR¶µ¤C?"ódÒl½Ñ?ÛÇ.JÉ°k?Å»Ý"L‰?Ü¡{ß¹'m?¶Z2€¤¸Ù?¨Ç—Ê/»9?œ–™ˆGz?à"ȓ›ív?¶)Ìsç£?èáÜu٘Z?£×"Ô$áµ?š¤˜Id,?ƒëïn	¸X?É5ù–ÚL'?¢Á`ˆÛû!MIXED4FGL J1755.6-2050¿ÑÞÝN,ç@'¹"ËÜãÀ9£B,Ë:&À:èî4%¡z@-=¹Ic@$ ]Øù+?Ã0ÞÖÏ/¿ŠSa?Ͻ‡?Ç×[†Žz?ý£øJÛ?îœÂþí±I¿á±—¢H"Ä¿ë7Rè`¸¿æd¿1ٖà¿ïÿþó…õ?ïÿùŸé"ÚUNASNone?Û¯±á‹R?Égˆ'Â? 3/ºïV?z"Ðïâ ?á$ôXP?ɋüãjóê?âq'¬äœ?Íi<FN»F?œöàDï`Z? ¥Nê^?Ú¯¬Å4A?ÌxÂo·Ú?Ý® M#?µ~#\֎¥?±ÔÃÁTV?žìE7ù‰?Þª¾ ç(?µ"|ÙäE6?àZ"O­‰³?²Mzæé ?"= ü7¿!?vÃá
+[?ÞáQOd(?²Ad"Î0?Ô¥qÏ%A®?Å6"o³í?¦œûÚɓ?¢'›îî%?äCwZnOX?Æ3‹¨jAè?ÔJ@.Ýý»?ʌuXÐ.?£\ÌUJã"?°Fý›ëÁ?ä¥#."y?Êë€y™_?Ò_šU'iá?²Um‹Aéº?²üÃlá0°? ¿odcm=?äpšg¨cj?³r}»‹"›?Ì4—'Ë?°Ûåê¤$í? ÐšðáÉ?Œ9#^À.ù?çåà˜Ëá?±Lä5!µMIXED4FGL J1755.9-4009?셕²ž<À^[ÕêÀ:'ci[ä,À;±£_9M@/ðÚs(—?üè˜`´v?ÛúgVPo?ä%+¾IÒ1@!='AŽ@@¡~O'7Ë¿ïÿñh?ïþ¦>½·¿ÝÇv¡œó@¿â¥ýàÀõ~¿îßô╋î¿ïÃÆ^‰UNASNone?àuV¹þœ†?Æ×°"Üb?˜¬‡3Ž*?'oõ'[Z?݊ŠXw¢?Æïá¼jvc?ä@­ÈXQƒ?Æϳ9±Z3?ž|nõÝæ?|Íò@î•?՞Œ¨D';?ŕùlúŒ?ãâõæª?³
3œ\?¼p üåCf?¥ê¤š›Ð•?ÒضÚáÒ?°
øµ~"•?äÚ!Ø~?°'ó Ê?¦K}¶Fõô?Im²5ì?ӂL˜Voñ?°ã9±ã£?Ù(&Wá?Å+÷#K½?¨ÚÒ¥•?£ÕKTõÍ8?áãï2t¾»?ÅâÄ2ô+?Úcx¾`V
?Ë(êk)€?¬™ä¸¾Ý?²Â/àÞÌ?áJhÌ-?ÊÇøzƒ1?ÜnÏ2¥=?³‡ƒóc;C?Ė—â™?®@,
F?ÙEéÐ~w?²«¿Q£²?ßÙì6™o?¸ï¶""'a?£Ð\XÏ?™ªörn¥?ݬdQ8W?º'ÞЖ—MIXED4FGL J1755.9+0953¿Þsñ¶®[@0Åè´k­À;\Þê¸À<·k;¸=@"6°î[¾?úA
a'Ï@ƒû¶Å$?ïEj7¬>¸@¡¥×•~?û´Ê­7Ü¿îÖ¾ˆfko¿ïÿë<ú\R?ïû!ô›?ïšT	lL¿Ýº7~œh+¿ïþ"?½…1UNASNone?ì,¼¼çÚù?Á'6ôˆÓy?ŒGgS¾q?¬×7!
ó‡?»-0Ý?ÀtãÄ3?ëôjMPÀ¸?ÌßÀqR[?±8YxAZ=?Ç,ñFÔ¦?®H¨9•Y
?¾s{Qî—?ë€I*ã¥Ï?¬:LQIÄ?ƒ*–œl?"4«žuì¬?ÀÌ:Ýçâ?«ZF¥.aã?ëþßs <?ÀqØÿÒ?gØòí?U?<7­[ç?¿RÊ<ϔ'?Àf—ë•î?ë@¨íå?ÂœÒo_?š:=e&¥z?¯ÁílFӎ?¿l,8˜!õ?À§ÆgÜÄ?é@
@B2?Ñݗ¢jðÜ?½ÀCçáP=?Ͷh<){ú?¸?#Æø…4?Áô'$D"?ê"]€—G¸?°õ•!Ÿ†?††Ç³G•?‡$#¡Çp?Æ'¥iå?°'c:†ƒ?çàÓEü}X?ÓÀ¨Â•ý?ŒE¬œ%œ?¶j€nµÝ?θX'ª?Ó2dôáÀAGN4FGL J1756.3+0236¿éP²7Ó´{@*áŒâÑñÐÀ:#}At>–À;ž³ì+6å@‰Àë,ß@¥½"J¥@?Óm©PÆÂ?Õ
ßâ©-
?ðßXÀ‹v@ÒU%v\?ïïB¾¤Ø¿è=-rH¿ìRþtå…*¿äÏ/!}¿ëðžc,ö?·ºú½Jù£UNASNone?ê^ êú<û?ºÛ
°»§¿?¢¹mq&?—³{Èg?Á× öù#Ë?¸×êáÃ{?크gÉà?²ŽÿgÍÆQ?—èZŒŒ˜?¿Nö7sB?«ú¾Œ=²?­ùlvÏ)?æ")dŸ´2?°pèflÅ?·ƒ¡
?ÿ?¤'H!έ?Ê!œŒ›¸?«@Ïr×Sˆ?ëú1ÓËç?˜—¯f'?–BNÇæi?tc¢.n"?ºä,s¯?–«Œk¿?æ}^ƒ?ÄÐÞÆ/µá?¼ýÅ&݇?¹ãåqx,%?Nj¿¯`ˆß?ÀMˆÕ[?é(Ȍ?ƶˆ«'?±Uì¼Cw*?¶T¡þÿ
H?ÃPi!à-/?Ây:Ú؏_?âAß×Ò ˆ?³)Ç° t¿?Ğ¢ïûóM?®Žtôƒ?Ñ,îØ\ÅJ?®â0†?ä*
H6?°ÛÆ­œ?¯™SB<þ?•´±h'e£?Ó‰YÂû?°m!#кyAGN4FGL J1756.6-2352?é":ÑHm¾?ÝÙÓÛߺ:À8"d鎤sÀ:/4q÷"!@ҝ{PƒP@
×^÷\?Ør³üœHK?Śx§0°ø@'Í|õôä@"\d"ä×?íQ`_¼(:¿í?½ÅGó¿Ì7¤/¿èpó‹(¿åôÑÞ¯xS¿ä@GƒLP;UNASNone?«•¢'æ³?¦2É`C¨?'2,þß/?'õï=·†ð?í½oÆû?«$"ac?·D!î?º8䆧Ï?¥ïªßq}?¤ˆaŸîw‹?ë¿ÎùÂ?½	fƈ?¾—›¨¬{?«ÅfJ8"?¾û*᳗O?©QöÓ펟?èM§.ÇW‡?±Ò䋿Ã"?´±NÌSÆ ?"/­E1³7? gû% …?…ö¶~wlX?ìh獵°D?—Ó	ïñS»?íª|¹ç?—¦ôÜ<U?‰Â´
?<óà¾Ån?îª J«Óa?¡+¬±Be}?¨r?ÔÕzˆ?ª¸rÿz>Í?©¯×ý
4ë?¬úž'ò?ìÝރ@Y?´§|õ>É?´žÚ">C?¡X¶äþÓÍ?½V㑊V†?©­‰™[?éÁH;Fì½?¯nFŽ¢«?™"›†9Ý ?¦²úCH™?™Rà‡º6?'dÔ"ÔÎ?îlT£±?"VÀ'Æ×OTHER4FGL J1757.1-1926¿ïêë¥øD@Ķ¦ڝÀ9±RÝóe¾À:þ»dÅ|v@9Xo­·ß@6¡|¼ê?Ñ"0?ÙÛ¡¦ÙH@Ž¨¿§J\@Ç²0¿;?ïñ1Ñ3cÛ¿åÏ®&ïX¿çÓû_‡O¿èÃ^¿ìr±˜"à¿ïÿï¤h)µUNASNone
?Á^hÿP‹;?¹¸¸BÒ¨?·PЕîº?² 7 0Tº?è¾K­R‰?Àыèô?Ý€òÐÜ?ÈMYº?·Dêcu@*?°-àÞE¨Ó?ÝEWotú?Æ/¼'|Ç?ÔÏÁÃH-…?²6ø¤;ë?įþàҜ?¬&a¯®?àlœc´—?³sû{©-?ÈÕ7Ñ
àO? ¹&õ\6?·à—\?'¤<‡[?æè±o×±á?¤1a×y1?¹qя»[?°Þ¦	±³?¸¢!šDê_?±x¨õÏqå?é¸
'å X?º¹Ëöl?Ɣj°¢õŽ?Ã¥	@_?ėíBÊ;3?Àð¦EIX?å4ê$³Ð?ǂ"ù"C-?Ç{àÁKdW?©:BñíÆ?ÆÝlúw?°."NAz ?äŸÇ˜QèL?´¸ŒRM¦?­ôHõcÛ?Ùvh5J?¹Ð=žàÅ?#+*Ì?êõ9]—`?¡—Ãm·ðEOTHER4FGL J1757.1-3554¿ï#æÕó£7Àˆ.D¶é6À:aÀ¥wnÀ<|Dôü—@º÷dP±@/¦¥ñ—?Ìr‰µJúû?á§ZS<=@áè¢ì(³@:ßý¥?ïþ¾°nÈ¿å$@ò8— ¿Þ`\̉°î¿ç¸A¥f׿﵂˜Ì@¿îñ›MοìUNASNone?ÛÖ+ÿü?À}D,x?¾j1°Éƒ?±–E™j´O?܏44~ц?¿ÂߎŠp?×ì3ÛàÍ?Ãe&Ka?³ð2K!~?­TJ<áž?á‹ßȹ(?ÁÙÀ{/Ì ?á1f\¼€?´äñM ÷Ñ?Ì¿ZsiO?°Y×e@ÇQ?Î|‹ó$
²?®eÉþÿ3ƒ?ãS¤›'|¦?¢+Ýô$p?¾÷69Å@?—¬œÛ·Y?њé:k¶²? M}9Ñ,å?ńa¨Ubø?³áéádò9?öÍĝ?·àe1O[Ç?å¾ùâ¦ö?¾°|'K|?ĞEÔ[É?¼qäÖ¦6Ø?¹Ñ«š½?µ…aMÿ'?çžJN¾æ?Àîž#/—?Ԏ‡\«&µ?³€zÄÚI"?ÕQF–^É?¶˜Ø)|o?Ö 2öF?³³9_ùä?ÔX®÷h›?¨†Ô6vÕ7?ÇÌ›,l?¨ž,¨äìý?ßÁEüIÎ;?­U'ât´MIXED4FGL J1757.1-2848c?Ĝ§±ñeoÀßOC427À9¸™9!ŠÀ;!-w1@
2AEÆ@ðÛâêE"?ɇø‡eºo?Ò¡ÿěÐÖ@	Gcä«æ£@«.4ä³?ïã²,¿Üáàš´÷™¿äµü¦¯,¿ç´<G®ë:¿î2BÝË!Ò¿ïÕ ÞœØéUNASNone(?ÂðPÍp6?º*"yd?°Fçf0T"?¦çÿ¹KJ2?é;ßÊ^?½ µ†xïD?×Zê®ñ+?©ó•ÆÑ?§
^†PÅ?ž3Íõ²B_?ââO¢C{?ÂcX]äü?ւ2­¯Ù«?²$ÃLf"-?¼æ	³õ?¤ˆÞÞð¿?á"#èM?²œã4ŸS?Ó'C2Q-?¢R†Qì›?¹G‰8áó?¢.hž$?ãS{7XÜ»?£Oè'Ôm?²-Ä.¼­¥?¤+»v{A?®(sx³ö?¤Nœ¿?¥Å?ë×ÀB*ë?°1ÓЋÃú?À¿Â­å?µwÙð¶Æ?®
« C?©I$;g˜?éïdœŒ¾?¹'DË ¢®?ÄK[àÜl?¦"ÆÝKTz?¾
 7Ԕ?¦^ÀZ÷?çGSюS?°*-·.'?»·ñÉõ=?—R`Êñ?À*Vߋ?šÏ╆Æ?è~lZØNò?¢h!'OTHER4FGL J1757.4-3125?à­÷"'äÃÀ«ºÅcLÀ9xäû—»sÀ;‹w·Òj@²:öËú@›´áô|>?ÀÁ_Eà´á?ÕàèãƒÈw@ߒޔum@_5¤ ?ïš½ÐZ¡¿ŽWÚÌ-¯U¿â«)yv
£¿æª)¿l ¿îà÷Ií¿ïòè ¹UNASNone3FGL J1757.8-3126?Ç×ñìÊvº?¶lmÕÈ(`?àùxT??ÄAËÒPð3?Óæp%?Á*ÑáoØ;?É}7îÙ¼õ?Àԙ¬±EÕ?дôɖ›?ÀW=0¦Ö?áF7Ÿ~Šõ?Â,žÜÒ?ÓS7…'q´?±ÊHNëxô?ÓÝj(4?²n*¦b?ØϹWf?²j]‹Ï?×ÑÛÒ?¢§"M¹?Ö¹O0X§?¤Ñȁ…óí?Ò;àôˆ?¤_ý¬Ñ?µXHC¨±?§´•nGÎy?⠁u
™?ÅT̘(?Öhûõ`?Ò©'"¦?´Ð¤v™Ó?²ìËyHgä?Óy±µ?Ưœ§ãUÈ?ã©h(ÞE›?Ç,ñïË=?¿P4úøH?¥/#/	Kç?؞ÕùFRu?ºüè&"16?ߍÇû›†?º [Ìý?ÀW5¿»¨?—]°0öE?àn¸b ¨?°V¹¥Ø¶?Ö÷ÿàÝ?®½\»nŠàMIXED4FGL J1757.6-2731¿ê¶I-¤·¿øÐÒëʾÖÀ:	 »aj~À:úÑ9C­@†"'&3@mâÀT?ÝlRƒÛlM?àëEþçÒ@
x¡UO¾?ÿm>ô‡|?ïó$Oj¡_¿¼‡!F÷‹<¿ÝA"Šfð¿ã¾¹ä¾¿ìÆÝ»²s¿ïïë€:ÕUNASNone	?˜¹¨$CMª?—U¨֏?—eep®O?'`'šêÆ?îï"÷P?¡cåöm?ÔQ€§@‡k?Çbˆ­°tI?£m§É?¡—¿I¸x?ä e;K¹?ƕ	¡]l?ËÕGâo)?­•9ŸŸGL?¾ÏHùª6±?¥ÿÁ¿ô?å0Å'`?±_R¢z™?Á%M%'xÓ?£ŠåõÞV?¦²Îsù?'?ÂSEN?êKÏ\ãË?©ãšŒ¼D?"}lœ²ê?‡‹3[»?¢]{'Ùf? AïÛ:f?î6?¼¥Ú'?¢¡ë'?»ÚÀÖIxD?·Ð>—üq¼?§2«ÚÖÿ?§÷ì÷iÍ\?ë}'6êg?¹™'?ùŽN?¾›ÄW?£"z?–€Ñ?½&=–ä]?¦R'Uÿñ$?è‡Ä•ÙË?­"§â
¤ú?©­|)»?•ÑNcQ?Ÿ¨Ïq¶´Y?–Æ8âàå?ígáÂ
'K?¢C=¸åg¸OTHER4FGL J1757.7-6032?ïý¼ãd'¥À1/ס<%JÀ:4Ú§€âéÀ<iË@ے@œÝ‰š?ú
¦ç_ö
?ÆÍÆó?Û]õ¿	j¸@³·õfI?÷Ïxw
#?ï×táSl¿âYbqå ¿Ó™û꽿͝CÝ¥b%¿ì}y¼"€¿ïÿßéà
UNASNone3FGL J1757.7-6030?˟Ÿûæô?ÉÎP
<1?åh—îô•?Ï{´mý«ß?ÀRÞHF¸?¿Ô`-½(?Õ!½ëïþ?É%zg>€?ᬵ³´*?ÊêÑD«¬?¾Z®Tð%?·¹èUª±Ž?ÐpÝGï,ô?°mý@zí?áù*ûE?³ÅYT\?Ç9™ƒ
)ù?¬PÈør¦?ÝÑU8Ôæ?ªxñx:¿¾?Óp_
N?­ ÕUºû?Í}™{‰?£õíÚ?Ã2ÀìøD?À{c²¾?çdçúê[?Ç´4§kX?Àpe¡MÌ?»ð÷_®¢{?ÅEµ£å?Ã{ Oˆ1?æÙþý²®û?ȵn¦Àñ?¾¤ž
$^b?¹"J	'ã¾?É=Èkàd?¯>z™a+?ã¦âù¬Ù?µ0*܈?È&«°l7?°¯tˆyFú?Ðßlw!Ÿ?¬?'kÖr%?ØXvƒêÛ¬?¸£^ùNyÏ?ÖÈó"Ç?³V~øùMIXED4FGL J1758.0-2953?ë Hj|öÀ0ÄÃéÏÀ:uK8¶ÈÀ<Tlô!-@-¡"¹ï@ÞZCBtð?Ò¥î[è´	?ïçùÿ4þå@U ÃÄæ?ýYnîöt¿îë\‡Ê?ï8tP3ôú?èëÏO^¿ã ž9%¿ï1…ý¿ïþ·á-VûUNASNone?µyQ^C6ž?«˜ö÷ç¯\?ÜÙuÉþ?Ãmì­ño?ކ§Ïg[Ú?ÃVBì0&?ªÞ˜•/?³"ú°#¸†?ßÓK>ö>?ÉÜ-äÐá?ÜÑ)á®cß?ÇwUÛîlž?ÎiHT=Ö?®Ù¦ÁHª×?ݟ‹Y¦î?´ö/.²>?Ó+Ð|Én?±`U
4?Âå-¶òoõ?¦"䚍¤2?çŸÐ"+7?³é§"3LS?ÀøSüã/?¨Rî3€´;?¥«ü›.Ž?›ÁIN.?ڑo§`_D?Ä'"19-?á\ˆbuÒ%?Ä7€4mÅÖ?™¼­¾ìCÈ?£)Üb?ÞÄ´@u!P?ÎuIZ^g·?ߟ€äA²?͑*ÌÔ¦Ø?¿@i‡?¦<ZØ¡hÜ?á«-̟‰?¸Q‰Äì,?ÔæŠ!_)?´Ö¸M­À•?®¦fA¦? Ž5p å®?é\»T³?¹u	.mÌ?Ãàôp™‰î?´
`єTMIXED4FGL J1758.5-3219?îÂÞjÀÀv–€àe0À:|r®sErÀ<
ÿ"Év@{Ý/E'Ü@
õ ¨ìô?ÕA[j	?îL%þpÛ@hò'hûl@Ñð~Ø£?ïÌù"@F¿àÓm›
à¿ÒjwØ~±·¿êìgpQ¢¿ïãh¬'Ä?íρ'¼±UNASNone	?ËXèø/.Ê?Á³òkúB?³S‰v=?®è%&Ô>?æ¿bð©å†?Ã(Ý؈Ü?ؚlM½?ÇYZlæÌ?ºgßjç³?¶é<øújN?àeÎñ ?Ä¿¯ÃQ£â?à¼ò;ò–?³S[ˆ" ö?Æ\§ÃqW?ª,<ëü?ÓWǧžêç?°ž|3Á?áUÞ]1Î?¯¶t%(Éò?ÌÀn¿AD?¨ô´öá+?ÍèÌ$†G?¨K1<õ?»qé†Z¼?¸'¾†Ó?³¨ùžmè?®ŒwL[°ý?êÍc©%[?¾+˨èõ€?Á5íUa?ÀGªè».¯?ÅP5í¢°D?Ãç)|G›—?æ^w/?j?Ƅ罶P×?Ó4ŒA?²eˆCP¤Ã?ÑÓÂ×¢á
?¶u@ªÝ?Úø›ÏÝV?¶ËìҎž7?̉´Ê!¢?­LÞÉCÕ?×]Øæƒ?·>λÈB?ÚôÞ¬?¶J²²*›EMIXED4FGL J1758.7-4109?Ýԛ
ô«À õìløÀ9w)@k*À;´è·äÞ<@´ËLD&K@³|™®'?´ËÞæ)ë?ÄxÑ¢õbî@
Õ¥á¦x¥@–'(6*?Œa¢²¿Ô±d ·¿ä€¿B Ž€¿àø>•'ø¿ê«ïxÉ?¿ïòÔÔK4UNASNone3FGL J1758.8-4108?àVr±?ÁÓ¦×Uøì?¼¾N¸Ru?±tÏ°ûâ™?ØÂã†ïë,?¿º=uxÊd?àÜ4}yí?ÇÒ²÷°óu?·ns4Cî0?°²!²6±]?Økú7q¹ß?ÆçÂL
?è¤L̝Ž,?¬è»Ëà£?´·mзÝ?¡±0D¿˜?Ãä÷C¡?¦	/-O?ç
èjfT?—­½›ŠF?¹ æˆf=?Œ€ï'‡?Çë3"?"ŠÜ¥M{
?С£È`pG?º[#<E*¬?È«%6ŠŽ?¹ôÃ?á"dζ±Ø?À)âÒr©?ÔFª
¢gÁ?Ȃ—8Z(Y?į¹*³?¿™\X¬¥¡?à°åLdKs?ʤñ£ç%?ãDí¥Šh¤?³Š9O¦F?¨ê`»p?¬Êÿ"wˆª?Ð!¯°ºÐÿ?®+ü~³g¶?Þn9è?¢²jqŸá?ÉÉ÷ߎà?¢ÂÍÜ¡"ÿ?Ôý•÷ˆ­?¤…Õå¡Æ>MIXED4FGL J1758.8-2326?ïø1q‰|?ÐÏÝMx"À9B£©½ÔÀ:"Õ¿º•"@ "»tৠ@Ö«ÃgÉ=?̕͜«qÞ?ÛG>©@åídòÈà?ûºouá\¿Üçòº•=¿ì½FA­?«ƒ¾ÆÎu¿á'§àÚ¿é¡!ƒ†Ý¿ïÿúÁҝÇUNASNone?¬:‹(S
ˆ?®¥³°Ö}ú?¨ü¯Ïj?¨Íô™=S?쬌[Ô£A?¶%9¡;˜j?²Hèü–.¤?µ¾EXK[ù?²äD\­(b?°>aý…ƒ5?ëZZUMO?»lUúĒþ?Ì) ¨m®?²m‰_–'È?ÉÀó?®uç`<yÛ?ây±ŽÐ4X?´|ä¤ê6"?ªÀ$:u6?÷ăc]"?«V˜'QŽ¢?'tÒ¿ôÚÚ?잔3dl¢??"qdè?{̀Öçô?¡™»>º7å?§å((<,?ª˜+W(?í•ÏO©®?±§VÏþ,,? 'hÚ O4?£Å±ÆnÍ?·"ÿÃËðz?·?aU¢¢A?ì‰y³A®?¹5tÃüw?ÂE6驯ð?¨Î€(ŸÕu?ËBËñIrª?°ÿm_´-Š?äÿIC7Z?³Oš r?ÁF<ít¢?|PZuiQ?¬žkZSùö?œ  þJ›?í°e–L?Ÿ1}ØFHQOTHER4FGL J1759.0-0107?绘gÈï¦@&7ÏÃøõÀ9Û÷÷oÀ;c§¹íÍ@ó!6Ü`@ƒÂ‡çÀ?ÍÃք´?Äï@£3?òãII.?þ\ÀJ]qJ¿³G'±Ê½Ô¿æ‹¨ñf¿ë··¶ùҿ絟=Ø©¿ïÿòɶ—×?î*éŸ¡UNASNone?íoëô–{"?©ká0¤;?‹TËUË°å?†ú(Oªb??±òJ{G?§µïÜ3"?íCß×|ºL?µý'ÒÕûJ?˜5èSÂÉ	?ž•?ßíP?¯§bžy¶?²mTUz'h?èø×(¶?¬å ›Pø?ªz©´+Ü¡?Îì
iQ?Ér5°À?© ýa>æ?ë1ïYr?Á?¢[£Vì&Ø?–Ze¥k÷Ú?{CeOÐûÃ?Àlõä?§'? »s[‡ß4?êfŠ¡a›?¹°÷ïF4?ªh³9&2?©(¬My¦!?¿—QU])§?µLæií3¿?èˆò…-H?Ç}ZÉ¥%?²|쾆mU?·f†Õï?ĝ¿Œ%t?«ðb—é…?ãîҎ¶DS?²btµcÂ?º9#'nk²?§OßÃë`?єý$û¯?¯Ô6¢?ã_H{€@?µ†+C¶Ê=?­N$üé¿?–tí"wٜ?՗ªhkEÁ?´xάÓuAGN4FGL J1759.2-0243?è¨~4í"@$¢hn~bÜÀ:cÒuðGÀ;ì†<Ń,@f°@O%'@Ó€™?Õól^MW?ïTów[0@ÀŸÀ$GÞ?ÿ=±nwí?îU€šÅÄ¿â;`"¾ŽF¿ãÝï3ÿáÍ¿ïH­M«"¿ïÿXJ?ïý÷ý}ÚUNASNone?ÉD\Ób	­?ÂyåÇù?Ê®Fu–kM?½ÏL¤×?ãW-ÁâÂ?Ê-ÆÈâîˆ?Ýà°ªpÃ?ÑV{‡Ù?Ö5½üû=Î?Íï~,+?ÇÓ"²¢Ü?Â8s6áò?݉ûìÊîü?³ž"ç¬lÈ?Í})E"P?°?·m°€¾?Ó·op®Ç\?²!9v†Sž?Ñ:‹-èh?¬'˜%ªH?݋ê§Ü°ù?²ˆd¡(ÿà?Ñ9Š)(H?¬,Cš1?¿÷–qho?ºpêV~"?ÑF&'¢?ÆJƒÍ»›]?ãjÒyèè?ÊöÃM?Ë@ôk;&6?̘ª< ?áá\-tÐ?Ñ28âI¶­?Í9$Œ?Æ®y¡<âE?Ó%i¯NÀ5?²o0»Ly?Ô¥s6ÙZû?¹mƒ:WuÐ?Ø5#×äÐ?·<	_y±?±<Ac?™uŠÐæÓW?âOZæLòï?½5/¦z—e?× ;"¯œ)?ºà¾
žàMIXED4FGL J1759.6-1850¿ãÊo7#
@îÒ£¦bÖÀ9'ÿ#a.À:ãóbb˧@•o¨@Ö¥†6æF?Õ/š¢X/?áþ¡ñ@XÈh¹ý½@{èP¶Ñ¹¿é¶V˜í!?ïûáÝÖ	Œ¿æ!['—¿é¶ˆRIxð¿éÀ¤ ^¿®<kb›øçUNASNone?æ<ppwÙ£?ĄGhÛqç?¶ô_Và^?±yEƒX"?ÌÄãÅ?ÂèÛ<7yû?Ï~¨x?èß?ÅÈ2D†ÿ?È
‹@²Å?ÁxdÔt?â³ÃT‡?Æ©Uæc?×-ŸöUm?³dgóf;?Æ8+¾ß?®AIC½Zn?ݶ\óËê$?³ÀwTbgZ?ː¶¶?£IÉ é?Ë¡^kè}Ð?¦5µ,…D?â3‡÷…³?ª|y¹"?Þóž'¨'?ÄãεÉê´?É+º}C?¾ÑEyÔ#Ñ?ԆÌ
b¸?Ä­'tÎ?¸8Օxó?¶Bîl»²L?Õò#꧈?˅U×o_?áÿÓWÞì¾?ÊÇPáïɧ?ÊÍUâúO?«Z:ûKJ?ËË}í@¶?²®Q×	¥?â†w§Æò?µŽubÓjé?«"}+ç?'3õJÑQÅ?ÒeÉ	ÁX?µÞ·¢?åÓ¨Dhv?µ"™"ú9èMIXED4FGL J1759.7-2354?î1Ƥ¦¿Åe¬­À8b¥)œ±À9™‡(}͋@ Ÿ:o°­@€ýÁ?ÎAN)Ø¢?΃*Ar>@€¦ƒŒçÚ?ûÞ?Þ½:3¿èÑÿ'›?çk<Žü‡¥¿Ö<×ÁóT÷¿áŽþµýþ¿êȸÀü4¿é–ƒ?4{UNASNone?Ír\9w?ƒµ¤çQo¡?'4…F'æ?‡>'š£ƒ?ïrÚ´Û®+?"ü:"»—?¤b˒•7m?­</^¦ú6?Â.ã@4V'?½Vä&å?ê.w
Ÿ?¿igÞDzB?²ë"\–dù? €÷ÊP?ÄþGæjúí?­f~n"™?èbý{@h%?°_O?ƒ¨z8§z§?kÞG¶/vð?ª¹Ýà/%?ÁÆ^s¨Ä?îÀ9I*t?'1Bî@?uyRJïä?{¾'ÅÐ/?ŒÂ@˯èÒ?'JÙUï#?ïbW†,]?—¢`EB²á?"=HšT}Ñ?œºã—ô»Å?ȋ7¸öMœ?Ä4ÒºÍpâ?é;GÍ&Âj?Ä{¼RÅä?±EÆ_ª?›Ñôe(_?ÇÌ!–¨£x?°
fÝ|ï?çêŽá|(½?±—Ý%ƒ?gÆ®rÀ!#?Y&Û¥o?­ëR•\½?˜ÌäÝöÒ?î	"/œr3?™<Lo@ëÞOTHER4FGL J1759.8-1250¿ï¹ã¼Ó@5Ïò=À9¸Ÿb0wÀ;A;ʸ@ýz¤6@ÝâïN?ÉÌ7;*£m?̱8òÔõ@ùæ
‹t?õ©%Lj½?ïöBçÜÌ¿çÖòU'¿ãêÕ+@«¿Þ]¨[ý¿ìÓ~AÏX¿ïÿð懈öUNASNone?ÃN2XþÚø?¸È޳ōë?—–¦'ÐF?'sž>a=?êo¾7øX±?º|}) ‹?Ø솁õõ ?ÄHdÞ&‹?¼‡í,Øj?´.í‡UÀ?ßñ–ѵ"?ÀÿÆ è?áå7^)ð®?°¿Èï|âð?´¸tÊ.Q? Œ"F¥H'?×tŽŒ?°S¼ùA¶?ÍnU̎þ?¢
Ô"Õ?¼òwg{Ëd?–úW¹ù_?åÍ]bÔ?¦®¡–!ÆÍ?°
ŸfC?§-ÿuI5Ý?¡7~æGĦ?›"Ó

¯?ìêåÝÑ=?®¯@rQzH?ÂAŒ3Ì؃?ºZXóÙxy?ÅëL L?ÁŽLSïÁ?åôÉí¶Ú?ÂŽz#)?Õo¥ ص?°FAâžQW?¿t'ôT"ò?¥Q'çö4T?áY¨q	ß?±Æ99‹?´|êY4*¨?•3ÕÇ&®?Á »{ù?£ëé(Ýv?é3Õt]?¨Ã³|!l?MIXED4FGL J1800.1-0323?Ø£m$×·@#•¯)M×#À9r•Q5}À;3Íw·Ò@Še¹ä@A#ßYw?Å¡«¡Y¢?Æ»Jî:Ü@8'¹ÑG†?özՖ´¿ï˜Ô!Õ½·?ëJþ€ù势è–ý»'"¿æªÑù\¿êLŠÝ"T¿ïÿö$´ë/UNASNone?ÜÒ>ÎiQu?É«!k¿?']ršþÓÃ?‹ò:ÈèaŠ?áõ?ÊTÉäm±?åáÔùÛ?Æ(û¼¾b?Ä;ñ»Í(Æ?½r²±åã?Ä<½ïþïÎ?¾øDèÅÚH?ãÙ¹òL³?±9‰ÌÕ®?®çº¥2?š¿M"ì•Ê?Ôo"Çf 7?°HŽð£_¤?ßGðøƒ½m?«Àf"Ü?Â!ŒÕïhâ?š®E»/P?קH›q­d?«š+6ZG?Ïô©é%¦‹?Á¼VäN"Ù?¡iHi·dí?›þ,ýJTH?æì@þÖgß?–IÿŽ§3?ېÙm*a?˲Ršy	ù?Ôx£(ÓL²?É»I9&^±?ÏíÔ¤?Äø'ìÑúß?Ü®øP‰/i?±ö\"Î)?¸"珦
·?¢±zò˜?Ý+ÍËqÐI?±ÐþH#?ѓ»¨Ê?«ÈÖ>­¾(?ʶôÚn1G?«ïmhf°^?àˆe;qI?´>ˆÕ:ÕJMIXED4FGL J1800.2-2952?æ´þ«¯À	³åZbL%À:<†&öÀ;Ðכ\è8@ü±A%@Vî#^©Ú?Ò2B…Þ?éC´öl@©Ì1œZ>?ü°Rÿ?³«`Á`Ýæ?îtOȕ/¨¿áƒŠc›±¿ê0ô)2(q¿ìÀØ7d\¿Ý@*<•UNASNone3FGL J1800.0-2955?³u;K/©;?§býX«?ȅQ²"A?¿ßŒ´Á?çp*9Âø?ÁZ»ƒŠ?Ã>U£ÿÚ?½)…ÊÚ¯9?Ð/"Š*«?Á¬‰
€7?㨎»*t?ÁÞ7i‰î?Ԍ@OÑN'?°kœ!D"{?͎Û"ƒ–+?­Ó¿¬¿s?ܬRìæY?²|u÷@ë?Ê­'¸4B?
ã˜kF?àœ¿ú_	Ù?ª‰![­@d?Ѷ©IåÒ,?¤Ã"ü3?¦d©"6Îá?œðÀßé?Ï«BF‡µ?ÂîO¤©Ì?æ®íÕ'?Ú¢«ï$?ªò¸°ëWÃ?¯'$Á‡H?Ñ´Ž+¦™?Æ{¬YöҖ?åv5»¬G?Å÷^J'k?Æ7a¯â3?¦'þdò¶?Ó»àæàc?·
m@ ,?à"7 —i?·'œñ6f?±P—]òR?e·,(?ãD]ÇRš?³F›" _s?Õ#š—<ê?±±s¾´HVMIXED4FGL J1800.2-2403c?í""æE*¿Õ¾¤žvÀ9:G#«À:A>Ž±@"¾]ž@zÑî0Ë?Ð輁ûî#?¤8ût*b?çk;³´M?ü@°?è‡G½-óX?ëÍGF®Ê¿éö;ÏÆ|¿äûñþ_–é¿ãMÁÔÌ ¿ágÑ­ÝUNASNone1FGL J1800.5-2359c0?}½!/óŠ?{|Û'ÐP?L5bo¹?O,êÒé?ï½~psZ–?|±a±}Àe?«Zoû!'?µ
Ú"|ªì? X[<í?¥WÄ6K!¯?íDØ?OSÙ?¸2‰¨hr
?»i'¯"¥?¥´ôfN&?¤`¥Ð<K"?—ÄÜ`"?ëLÒRëâ?©†sòÍØ?¢-®öäR™?†t+Þ;?"Û!Át>?'3s'!iØ?î<æ7¬ê"?µ÷s>'
?'õN¶ðå?‰:€•¢Ð5?]5݌¬ƒÿ?Ÿ²6B÷?縷ô7''? Ë"±NC? ãY_¥~–?¦®}'²6Í?¢ôê?|×<?±-µö%ï?íÂ{ÅÉ"s?´§žžsð~?²Sð®Æë?ÅÝaéZ?¢\¸ØÒñ?"ŒÜiD^¡?쏶`©?£&—ýë?†PþÞ€Õ?urã«ð6?'ø½–xýÃ?¿ÂH=?ïöýU^?é.ó¬ŒEOTHER4FGL J1800.3-5237?Ô6"ñÀ,!ámmÁ¤À:óp–kðÀ<jm³aÁ¼@õ^£ylS?ó²õú:Ä?ÚsW%*ÜÍ?çZ)ûÒ@p¨ß‡ºt?ýÒv发X?ï«P°ò{³¿ìi¹Âƒó•¿"z±ÄU&o¿Ý#½¿"©@¿èW B•¦Æ¿ïÿ¬óéqHUNASNone?ìŸohåê?ȳŽ19?nn Âg?x¹–k8D?¾šÙ^ ?ÈÉú†)¶n?íü<Ç0«™?¸ô	>ק?†Õé"´?—¢>P?*?ª†ï'Ö~=?¶áÀQ2Z?îð"g^?œO{ºÍ?Œjd"?‡£ÕBù5?¨ì£CöÖµ?˜†L;Áù?éV²Ý@"?¨´ÒU?'*àZF"$?zÞCTW?ÈØßV?¨¤7ZÉÊñ?í·vÓU|?²mi\Êb8?"–']x¿?"K‡¦q«(?¯bî9hˆS?±ÓFQ¹j?ë²/ÿÞ#?ø¡Wå*x?™€>´Áõ?¦ýëÞÍå­?¼pVæQê?ÂQÞܑ2d?ìãh«Ì2?¥eF¥²ªØ?'ïVñpŸ?-ñiŠ\?¶õ(åS5Å?£{rŸ×6¸?äàXvIïs?¸/SÏðJ?tX^¿<¼?"¡¸Ü[ß?ÕS¬P'¤?¸mä2Ò·´AGN4FGL J1800.5-2910?¿‰òwÀÀ`¾¼hÑ{À9"ùdŒÀ;æA@9
6u@¨âù3?бuBø";?Ԕ@~Ë7 @]›¡±–?û÷Zþÿ$?àɀ2Wk?ìùŽâ0Œ:¿áÑ>vˆH¿ëGÁ	Ë¿ßÛÄhû¿ïþ)›Ú¼zUNASNone?ݏ×ô?nj]ñ͸/?¢}‰
Ìß?…ow#{o?àN§ƒð™?Ç©|ZïdÒ?Óóì©ê}??Æ2†¶¤'£?°¡ÞãTí{?«>Wí`?ãñÍλ '?Ä>ócm`?Õ¼ò;h®7?²"ÕóT/‰?¹­]µ›e?£tÚ
m¯?áëÛ,$å×?³"^¦ËÓ ?ÈúúXÁ?žå£"ay×?ÅPŽñÑ?¦{ÖІÀ¤?äm;ئÓG?§åRœ±?ϲžò¸³?¼[S–]­Ž?¨TÌáÊ©À?¡DA+!'?æŽuBæô?¿Ô\j?ºÊ­<''Z?¸	õAù=?·µƒCN°Ó?µââ9çš?é¯ùðqlª?½hLªÖ‹?ÅÅÀ^Tt!?¨*
<Bš?¹G‡§IrŸ?£Þ"ä6=?çežóÔ+D?°	^ù_¨?¯žݘ?Hûs2ºƒ?È|û&Ñë?³x=Cü[?çïP°Ð›?²¥ù™‰~nOTHER4FGL J1800.9-2407?íeÈm¯¿à]Ÿ¤u–À8DAYA»À9Îb뇢÷@ ì1"‡c·@Ĩm'K?ÂÓÝ7S(q?ÂÏڞF§"@
 ðbÔ
¯?úo·UlC?ïÿ&@±v¿ì§w¨®	"¿×
;&òˆ¿á¯`«;'¿æóû_‡O¿í¨]»WUNASNone?©Â¿F–+??¿±çF(a?†_ãλä?¯K˜ÀçÍ?î
T|Pí?¿ñ·<íœ%?©¬Œ;gS.?°MP¢98K?´Ýã]xz?±3Äéٗ?ëã;™#Ž?·SZ"¥?¸¾Í³6)±?¥I|jÝú?À[×íf?ªEÑ«ºËœ?èãSðm?°Oš
)?ˆö4µAÕ?oºÝšÓ?¤ºógˆ}Ò?ˆzŸÒoƒY?îPx¸oêì?Œ	öúël?›cö×ú?´OëÀKí¼?Š"'~bö3?"/?;\Õ÷?«²º—?µZôùSÍä?™º!üŒ‡? ŸªÔ?º`[E²"
?¹Ið`'?ëæ#‡2}š?º%xŸ¨?´çÜõ±>ô?¡¯ï"ÃŽ,?½Ñ`<šÕ?©ayØ???é¨Ø]=Œ—?¯ؙ—gÑ?jIÏëYè?YQ´{èƸ?¨­ðürzó?'ßëòÞ­–?îZ¡¦zÊï?"N΍OTHER4FGL J1801.0-2802¿é"	UÀº;<ìðYÀ:+PâÌÀ;¹ë1;â.@÷§kê4@Ôef—?Ìô¡}Ð<?ãÍ?ïXz@¢G²?ÿÝ#?_¿ÀçÉ'{Äò?﷙ÊAR¿Ýö5{âÏn¿ç5šìð¿ïâ&›u;ì?ê¯òkÂƺUNASNone?¾ŽÚ/Ù-ü?®»6MI'õ?ƜŒ
ûýM?¼!"xäÜþ?懶…Úí?ÀËMªÇƒ&?ʿś]Ǐ?Á>zaùwÙ?Èv·Ï1""?»ÍêTÙ1p?ã2`¥\E{?Ân"ÀÊi?ÑhØ[¡;y?¯]gñ=?Í·'"kV?­v=Á??ß»^Y–c?²·Ô¢Ú
"?Öf¬ìK‡?§µ"W,¯?Ó^7qÆ?¨[¨†¹K?Ö;¢¦f9?©µò
¹‰?«2àÅ*« ?ž«ê´QF?Éæ"z9"0?Àx©èyÚ?çÓITÌyÚ?ÁVGÆ_˜?° âÎ(Ýé?¯°ô2¥d?Ë[pò?Ä̃™Û'i?ç9Éð'?Ń×e'å?ÁEó+}©›?¤ ("ý'?ÑÅ"›Á×?µ©¯¦Ì2?âËò)R´®?·^¹éY?À`àË1l4?œré—ãÕá?ÙWï×$$ß?´s¸¦¨Šs?ÞwŸÂ0DI?´jÓ«µ¼?MIXED4FGL J1801.1-2626¿çE+øΪÀ¿û,0ªÂ¶ÉÀ:X`£®ÆRÀ<5ßüTz@ k\sÉPk@DR´Øº?ÒիÒ¼[?ïكÿÔa@þB҄?þ\×w¬	?îŠ<d4\ÿ?ÓÔ
c†7<?¶ûlâU°¿À]6fïMU¿ï€¤ ]Øù¿ïö-ƒÆÉ~UNASNone?¶åiE²"?®–dàô.ã?ÙïGÌ´?ßòp—º?à+È8úƒ¥?Ãj—îž®¬?£ü
º'?¬Z¢úö"¶?ÝpobÓ"Á?̬íîIc?à±
Ç?ÊÅÛ-°	?΅e'?®­%ÍÐö?Ýõ
Ê)?¦?´Jð
­?ÒÈb¯Í'?°0âÂt²™?¨¨ÞUR®?"zîË´¥¸?êÜHۑ
Õ?¯ãhÜ¡?¼ÉIú8ځ?ª
æû܋°?¦' ä#? l}}ju%?ܒݨ<I²?ÆD¨Š''?àUÈÅà?ÅìÆýªæ?Ž+0_<?—Ù)ÒaaD?ÜÏå¶R·Þ?мO–á?á`cJ°±?Ïbj©þ&ó?€–%ÏP?¨ë%"Ze*?âËúÈf>?·òãNâe?Ò¸÷‡‹z?´ìZ¸†?ƒX\ŽÔu4?~¸ââY}?ì'åOÐwÒ?³(‡š;ö"?¸ýÉïÍ­È?²
ùƒË7]MIXED4FGL J1801.4-4307¿ëµ!ÒJÀ#³y1DEªÀ:Tb(êÀ;ÛüwµCC@½±$¥¦Ã@œ˜D/ú?Ò§›ûH¶'?ÖáUðÍ]@UÆ2o?ýL…>õ?ïÿÕm…>™¿Û½?¼¥!¿å¤œâ¤O€¿èGGÝdI¬¿ïÿþÐñ?ïõv'[¸UNASNone?Þ,<kbœ?ÇQ\¶[¾? }'Ó?›ý€_;ç?ßî1ޖÆ"?Ç"j'^֔?æ
äå>Õö?Åí(¹ÿâñ?šCkÍt?¢fÓ¥'PÀ?ÒB!þW‰T?ijf²š$7?æ&"ðÕð?¯¾–õ—Ÿ®?²^ËÛÖÂÿ?žõôq(!·?Î6JR<@?­'A±|ï}?éhsÿè>?¥Q{Ód? 
Òbpµ?ME?f©?Æ[;ž¼™?¤BÇsj³?Ö¢Õó<"E?Ç;ùùs?ªÿ
ŠÙ'?§RŸÍÞ?âþ¤-Ïϔ?Çq¨¦t?å?ÛPðâS?˟Î5œ]Þ?¬LÈ^Óô?±°L>–‰?à'»+d²²?Ì*ÑîRa?àù¾z`?²ÄM€8
?¼\Ä«Yú6?¤£/4?Ÿ?×a\´¿mq?³6©RêË ?á"Ïu"H?µ)ž¹R?«fw×r°0?•Ýë5—?ÚM'°k©?µ-|¼0uÓMIXED4FGL J1801.6-2326?î°Tû¿Ô,™î˜ÏÀ6À.¬»µMÀ8óq}ñg@bQ#35â@IN…Ÿ?ºÍHÁºË?ÔiQÓ1jÜ@",pCß?ûøúJ3ß?¹Ëw7Dù¿çõYé€aº¿Ùk	ä/iû¿è\ƒ3&¿ê˜È]ý6L¿ïý ½é¨UNASNone0FGL J1801.6-2327?Š	ûɒð-?®8=ë[?ꙶ©ŸÌ?ȶbvÙ?ÃúágäjÎ?Ç~PN2NB?‰*ì~0J?˜aº¶óè2?âusá	€î?ǖ8yvÂ?ÚKÀÚóx€?ÇYxR:?°28\Hó?¢"Ÿ¦ñ=g?ßú˃	?·nqao›?Üè[¸QY?¶þª •á?9ÈË·whù?%¤Þþ•n?Èå
Aˆœ­?©³ÄKˏÉ?éÄV2Þò?©¶˜÷a?—ôVy ?»Ñ‹ùGÿô?è'&·'?ˏNI¤Ò?Ì«¼á7?ÉV;ǒŒp?z+û¨Íß?‰d{lÂQó?ä"&eøàÚ?ÊÏ]–?•?ÖoE&G4?ʨCDg&ï?¥è»ãíæþ?§Kâ@LW?àê¬FÍøO?º?nß?ÛmöÏc?¹iàd‰`t?&ŸôBÔ?[‹0˜?бSf¦Ê|?´!稽›N?禽L.?´"
4à¡/MIXED4FGL J1801.8-2358?ï€ä•Qœ'¿ãŠoŊ¹,À8''Œ6À9îC–Wź@!Í-Ŷ@e¦$ÂW(?¼"T=ïÐ?¢¨süüë?ñä¶Î]Ç@W``u?Áüža)?ê¶( Þ†¿äµešŽŒ¿åAÍÊùö¿ç™§ÜR{οݡ…Æ}þUNASNone?­-sI±v?¬zh1.ے?ƒf~½‰Þ?¢A˜Lxº¸?íàó-ðºN?°êóÇÙ
,?³Í"®1?´í6©©??ª®ë?¨Ïhz³?ëåD‰¶'f?¸‡_q‰íñ?²bÆKbÛÁ?Ÿá³
oIÙ?±'å9¥õ?£?ïæú—Ù?ëjQ'v?¨¤õê?¶ñˆ‡½<ü?—f{í³¸"?¦ÙžcÐ+s?ˆè
Ok €?ë´5ËU©?œ0òû°q?§ÑgÛ?ªhmŸ3[?ŠË­/Q?£w}cò²?îºÙ|ªî?°Fϗ3a!?¦}ˆtöŒ?¥Ø…/ßÏ?­Ï=S=VÝ?²A`ÚÀ0?ì»3¢X	?µ¾u•/1?¯DNˆ€?›†CésR†?±Ҕ²¶?¢° mŸ®?ëé`Äïf]?§µj'£/?¢dX"«R?‹Ì>Íê/é?«\™o8ƒ:?"׈í˜×ú?í#ðßóèg?›±Lt«OTHER4FGL J1802.1-2652¿ì3¼'Úø"ÀÛšþôgÀ9Ë
By!TÀ;U
×ÊVÑ@ù
ö¸®ˆ@c4ÅÚjD?Ì/ú;É°?ãA³ß@ñ@ûÍxÄ6ü?ö"Gx¯p?í¡ƒræ§i?ï5+ÆWgÆ¿Ü2+`ÖÚm¿éNÜd…¿í/êß‹4¿ïÿa>ß8àUNASNone?³^&?d«?«š•A@D?ßÞYˆm³s?ŗTM'¸‡?ÛJô'sb?ÄRDìÌû?²(Ö@œ…æ?´p­ßn1ƒ?ÔÅà"ªÇi?Æ.;Ä?ãWô헏?ÃÞggJðr?ÄäýÉ=?§ÓèèÜ?Ò툓%Ðä?²{P®?áP
ÆúÈ*?³HNqß,?œ_×Sߣ?z™÷¤p?ä)֗j¯?®È藧¨°?ÕæUa'ڇ?­±{¹dB?›Ü€1QE?ŽÙÁ%Du4?Ý­4vTE'?ÄØjZíŽ?àJÃ[R?Ärý9¶I?˜îÐ5j£•?¢#áO?Í?Õrh3+a¿?Ë,e¹˜<¢?äUdzAÔ?Ê;Rw­FÜ?µ–íDv?šjˆ»Ï?Ó[*p°±?¹u+'v?㟠Âí–?¹vñs×/?xýZµ‹n/?b/MPbêk?å§)£x¦Á?³Ì–…¸È%?ÔM·M´"Æ?³"ˆ+R×"MIXED4FGL J1802.4+3634?ïé_c›c@9
TûÚ×RÀ;®ÉÀ¨ÒÀ=L-·É/‰@<# –x}@©Ã}˜²?Ô¶Òd'O?ëÄ=aŠ^"@£ñb®K@k
>pN¿ï Å®?ïýáý¶y¤¿×6ÿ[x³¿æ`¾ø¿ë)ZÖ¯O¿ïÿô!O…úUNASNone?àãàãì4W?̵"S-ÆÚ?نåV`1?Ìüh›ÊÌB?²ÅcˆŽÏÿ?ª~‰Ò4k?á'ÅuH4?Ë z|{"8?Ø*ñeˆoü?ʧ¤ÀÓè?¶à$?}Øï?¨þ‰éenK?â]¼Yô#?´fÖ®
Š?Òcj'æùÊ?²Ìk®…×?Á3´¾Ê;ß?¥DtÇNÉí?äy°8¬ç?¬LÊ	Ù/¢?ÕL÷KóÁ?ªú<t4I? Žk6['?<ê˜ÄðP?ÚNæ1ø ?ÊLÔ]ԋL?ßFKF'ú?˺°°;G?ºgNNôÒ?³!›ÝËà"?Ò·RWKý?Ê¢êGÝ?⽉#äû?Ìð…Ûˆ?¿7Eš¨0?²‡Y«£út?ÛÇœŠ»?·u€(O£?Ùûí­?ºrd:V?Ä{°œâƬ?©Ì:'g5à?ÔÎUì_~?²[Å´MѤ?ã"zL'?´;¹]$
†?°£ØB
ûó?¢(Ÿúdh=MIXED4FGL J1802.4-3041?îQurÀ3YÀ+"¼ÃjMÀ9¢{oâæëÀ;ÍÑÑ‹è@dÓr®HR?üېIŽ¿K?À¡u´6S?Ö
´ôhó	@åB˜I@†â8™Ït?ﯦ¶¸ŽQ¿åé,êCÖ¿Öl^"9¬¿Óoô¤Ø$¿åÚpú>¿ë©ØÁw¯UNASNone3FGL J1802.4-3043?äH}=©"ö?¾eQŠÙ…?ÍnÈ0}C?»«;$Ì?ÁoöA).ç?­,úœÚ9ô?Ø7
\û¦?ÈAÙŔÛU?¼*
…#ÀÏ?·>>¬‰<?à_7Å-
?ÅÃŶœÎq?àß®j¥Õ?²aÌ`áœ?Ó>0ÅÎ4?±ýFq'X?ɈæïÂ?«'ìh'?âLÑ6`[­?£n££ht?¾KnñØÓt?•ÓY›â%"?ÓӁÖÉÉ?¢?He*™_?ߋ«Tµ˜?Á5XɽJ?Ó´€þË«?À«˜_1é²?É©™}%?´s[œà^?ÄÚÇ%1ׂ?Á}—@µ
$?ÅÈdõ7>?Á‡4^£Æ¼?åW56v<P?Ź÷
¤>Ÿ?Ûêô
6'?³ªÃ/Ê[?Õ? ÌÔ.–?³»`üÍa?Í«ÖKëT¼?¯Õiý•Y¨?Óñós×?§?r;ËL?ÇÊ®$3?©'1|Gü?àZ½»·Ò?¯˜£CtEŽMIXED4FGL J1803.1-2724¿ïÄ5a`ÃÀw_}>@À9m@wÏDÀ;÷¹à`þ@4úXKE¤@·Í+d2?Äé‡B©ó¯?ÐTÚ¢ÎL@Jd`Ò©@\+ž>nü?ßeˆÜ?Çõlh³ó¿ç'•`$¿çÁý &¼¿ã.ÕÖ`ÊE¿ïÿöàœjUNASNone3FGL J1803.1-2728?ÙX܁?ÆÑfôo—×?©4,
'©Æ?Ÿ`ž;Äñ?áÀNþÚØ?ÆËÍíÍè?ن\ßî¬_?ÄÕ݆r9G?¥K»œ!)? "þÔr7Ê?áë|Ôx#?Ãñ$e:|?Ý,>Àb¹¼?³[³G$2¹?·Z§¼®-?¡ÚL')ã©?Üý:®¹?²ÎmK\õ¤?ÕF™rz?¤°ŠWúkU?µMäëJ½ô?Ø¹¯{¾?â³:[èÄ?¤Âk'"Áq?ËÚ®Wæq?»à°*c^?±ž#
˜'S?¦…qÔºŸ&?æՐ‡t9?¿r™¹Â?Áûûׄê>?ºÛ.(K=?­íĎf•?­j,xìÁX?é¢0ñ[ç?¼±´B'KÇ?Ïpp4½Ä?¬Ÿ™àþ?ºæÑÊ|TS?£¾ºÀy»?äÇ%ª£F?°L©Ðá?¿xFÔ¤²?šø"–q'?½ Ù-G$Æ? Ž¬G¶?è\ܼ†Ñ?¥]òåÎMIXED4FGL J1803.1-6708?ïÉsø†u6À4[çÈіÀ:èÅPØÀ<Rdë<#@ü:à>Å?þ߸Í;‡–?º†ÕFÃÞ½?Ð,âxY@|¶"‹ë[@à[8Šàï¿æË£¢1пۮ!æڕ¿ÝW˝>?¿à./ˆƒÇ ¿êÜV|E¿ïÿÿ&¦³UNASNone3FGL J1803.3-6706?í1ú¶6»?¯Žf_°iÀ?³&Žï
~"?­,+ŽPþ?ŠLÚú ?²ªG@'?î Gn\1¸?®ã囏bë?"NÛúÿ?©p
x÷S,?—¨6?'!?•_]"¢è7?é#™
085?±P´þmça?ē½ƒ?®@¿[ÅÞ?«z$c€±?œb'x@Œ?îŽþ
1‡?"W<ÉÕ6¬?•ÁÎÝlXù?tÂl" ²?¤æ(¯ÊÔ?|ùXÛfµ?泀b2q?Áò#š6¸?Ð
Ljø؀?Á—q¼­?¤u–†Éñ?—ì•êãc<?ë28jÓ´?×J¹%"Ô?´ÐÈêF¹?À¹ÃE9›?±s¿é…,?®}‰Ö|%?áäçÍÑ|?»n•›…ï?ÖlN°šÅœ?¹È!p¬Õ$?¸1ž(+?£XC¯tz»?ëZ#än?H¿0Q?¨8TQ³Hd?¯8;S?¹¤·)Ù`?"å#ŽX%AGN4FGL J1803.3+2425?ïHi"lƒâ@4ðx…LÛ{À:SºÜ	€²À<
A¢a¿@#úVå@¾"[Có?Òñý=­àx?ä㼝ª R@™Ê&)_u@¢+'ôØ¿àí0_nO"¿æߝ‰é"¿ìùXç!â©¿äŒpPÊó¯¿ï½þž0§¿ïéÜ»WUNASNone?Ùêít?£gäPè?¡\̍ ŠE?¡g__¶õ?"e—F¯ì?…fp'&rI?æ}¡5;Ãr?Ê/ý¢òL¨?̾1ö¿†à?È¿MCà?²–'e3:´?¨‰¨‹Î ?è^6Kìg?­D©8?µåÙÙ»?¡Ò£Duø?Ô^㠇p?¨ˆ'öüç–?èî‹&»‰?¦°©À(/¼?Ã}?;)KÔ?¤ÎlìÍ?±'(Õã×?ÓªÍå?ëëe°€Þ?¹õ"¡z<?¼ˆ{úwTö?¸_Ø❌?qo¾ZÂd?':ÇýM?Üî«U?͊ÜQúô}?Ü	Â3õ-?Î+êmáHÊ?¿ «yÉx7?²ƒ­©XïÔ?䵗ԝ{¦?³¥I4¡é?ÀêXÈ\êV?¨Ö=Ž–?Ì?Gå-'?°6Ö«ZÒ®?Ý ·'–P?¸j	­©?ØÙhs~IS?ºv÷\‡.L?Ã
#©þ@¸?¦ÙÍlÕ¡AGN4FGL J1803.5-1639?ïÇ_=äMX@,ئãÀ:"¿Z'ÈÀ;ß[.ú¿N@zƒEÅ1"?þ­<^Uí?ÙÓ»¾Ýuç?ïBR‡"Ä@¥b?8È?õ£Þ&;~?ïí(Œç°¿ç|˜×ÒºM¿à±Èà5j¿î'á@øÔ¿ïÿÅGMƒ?íaâ"oUNASNone	?Ëj¸R
á7?ÆxPÍç˜Å?yb¡È­§?¬{"É'€'?è9†ÖÀ¸å?Ç¡çvú¼?ԀJ"Y'?Ò}ª.¤ê?Ñ6?<Uñ¤?ˏŸ<=??ÚIv­µ4?Í F(z¿Ü?Û¹î×AM†?±Ùô¨úv?ÉÂA"{ß?¬drÔàvá?×dð˜a"Ì?±+D%™£?Ó¦¿ßué3?±n<ønL?Ò´.xìÙ?·ÙK?Ú<‹ò)ô?¸Vð}ô%?¼>–éý¿?¼Àñ',+?A&p?Æ?¥ó¾œ§?ëŽ#ïíš?ÀCu;§‡)?¿©ÃjDä®?ǏûõÑ ?ÕÚþ ¦Ë~?Ða.OY?áHBcý«?Ð$ˆX‡3C?ӖêÕ\¥?°;Í=cwo?Ðå4ïî?±ÓèrÎ1Y?ÜLð/õ³m?³­·!®•?Á~*°á<y?«'‹ ŒÆÛ?ÐÊz=™ú¤?Á²È"®Î?ã;84ú³?Á²8ržiHMIXED4FGL J1803.7-3207?ÞÍ[Á–ÀâP.ì|•À:
5Ä+mÀ;ó`µL~@ŠŸþ…,@ù×Vé?ÌÍ£6{g?Üp¼`mþá@;=ïí™@ó
Ýԇ¿°žaÕ]-?—B&rþ¿æÛÆ/#Ùú¿åÚv»œ#¿ïü`Ÿ±?ïÖ¢
±nUNASNone?Ð5IÆÑà?ÀY²"C"?§êë'ç|?¢"Ãz³?æf¹ÞX?ÁßlÍÛ?äŽåØÙÃ?Ç8ºº.B;?¢ò¾º? ?Ÿñ;N!Û?Õ½CÛ ¨?ÅÃ-m1Â×?â+úè?²éOø™aï?¹INtúuI?£Æý°
‡?ÕoVJˑu?±¢ì ì?èº(¡Î‹-?¥ßîs­Ð?©0>5ù.?ˆ¡·þ½x?ÆËMóË5À?£
Àìì=?»Â´^Zå?²ëį/?©äL4$ä€?¤ÎêN"Á?êéd¼±æ[?·ö½ð'>?Ôb¸¥2³?Èyʯ™¾¶?³ÐžÏY1?´˜ÃvÈð[?ãT"y³¹ð?ɎwùR?ӏÏÁHà?²8±×þÚ?¸æ»áB?ªz‡¶'MÐ?áõIÞpc??´"Kò‰Ú;?ÞÚ§é
ž?²Ô­?3‰ª?»¤@Ò@Í? B§ê?Ú<Gâu^/?²öŠO«-MIXED4FGL J1803.8-2908¿Ðm…òü?	À[
Ø/×^À9··ä|À;UûKeY @X4Pi¥@(©6Ŏë?ÏLáÚûä'?íÕ€ÙÚ@Uí¡Xª¼@¢ŸÒ™?çˆ]‡º¿Á":šZ´¬¿èœRnM¿ìz¨<ʋª¿ïÿ¹ô'ô<¿ÞՋ¸/‡UNASNone?ÀùgüNÖ¹?ºÃnK¯x?â.¢¥9"?Ì1r0%7?Ó'F¼Ž!}?Æ|ú°Š?À.¾´ŽÆ?À¢f°åx?Ù®ú?‡æz?É!€g]K$?Þ9¤b0²á?č4yŒçb?Û¿¢="D§?´•63àی?ФLƒ'E?±§Ÿ'B?ӜLué*?±'4™…e?¥ÇdÅ?ƒ¼ÌÙq¯?åØü¼S®?ª¬­/"o?іóšt"ƒ?¨È¾Øì¤?µ5ó2±?¬Q"=ˆÞ?âÙ^
&"#?džNÛ|µU?Õ©¦µ"?Ų°rà.?¥ÚJY¬?°Ržî¤*E?ÝÁëq ?͛¿I蒌?߂ӗÊÀ?˯8‡…ðÅ?ѱ@wÇëD?±‰²'WQ?ÓOº–ic?´ML>܅?Úÿ¤Í¡«X?´É­‡å?y!Ög}Ï?dkŒzÖ´?è¯9`ô·w?°ÀÖâ"î?ÌzÌ^_S?°qþI¯gMIXED4FGL J1804.0-1124?­r/ûQ@r€Æ^À:)vþUÀ;ÇáR•Ï
@D•pÀ–@Ê)"]È2?Ñޘ\Þ|?èd÷eýŠÛ@•—'$@8 GÉa?ï69bwCƒ¿Þv¦…:g¿å
¾"Š"¿îp;Ñg¿ð?ïÿþˆ0»ŠUNASNone?Ùëí…:M??ÊGáË·xþ?Í-Ò§"hŽ?ÅӞžÍFV?×})&ûþz?É©h³a…›?Þgš^÷˜d?Ç';Ýj˜"?Ä¢P]¡­?¸ÎÿíΊ?א"yìw"?ÃÇÃÅßj+?âô¯Èb¸?´m&ÙÒ|Œ?ÉDÙg©¡=?± r'9k?ÎsSÙ4Óá?­¦g="î¼?áL=LÞø@?¬Ül4Ù?ÉL\mêË?¤
—J}7?ÐÁW0ÆúÙ?§%,u®÷²?Ñ££Õÿó¸?ÇT©S0÷?Ò'R€Þë?ȾƈԿ#?ÜXÊ×-]?ËdÀÃmí2?ÉU¡ðÞ­~?ÄU9å¡Qk?ÓСQ¸ž0?Ç×Bý*¸?߄¶êëÏ?É!=BçÂX?Õó'wñ±¼?³ŽÀ|ÑD¨?ÒÀ2cï,?¹9Æ'?×L¦$!·?µ0­Áː,?É:›B¢M?¨~ÆS'Ím?Õ¯—*\'§?µ5XƒM«?ÝÆK‰gñ?´[u ÝRþMIXED4FGL J1804.4-0852?æú_]Yó@ò[1~þ
À8ùg+ˆDÀ;	q(aH@~öº†ú@¼R?¼©HðÕ?ÁØQeMa³@›ð™Z¯y?ÿªñ=D"¿×
P`½§¿ápv̗¿èÆ6°–5¿à½!=èBõ¿éþ=½Ð°‡¿ïýtÀc‰UNASNone3FGL J1804.5-0850?âãØ,?ÅӐb…¨˜?¬VMt^?¦Q…+>f?Økò÷·e?Å:ºÄ•#?Ù«ÌÚí)—?ÄÆ (r¨?èÞÌ岈?»Þ]ÚÿY?ÜþŸý%?Á?½ý?ᛱ›æGj?³Ë©ô‰	?·5•qÃq?£IE3ßØ"?Öû7l0ˆg?±óiãMI?ÝæDJ»C?¥'êh‰ÄI?»÷QŸs½?"Ә ¦?ÛíESØU}?¥‰zåè?Úg¹9iz?Á$Œá>7¸?']¸q)?·¾ï`íÍñ?ÜO—êLÜ?Á={@h%?Å'?~'?½çbËYý?Ϋ¢	œH?Æ;S8¥þ?ãG¶šRÉ?Æ5éG?ÙXf|l?³Ø3Ä?¿2'a¼³?§1k'VP°?ÞÛ"g?´Bvá_‹>?ʉr5¼¨?£ç(ϟ>?ÇÆF]â?¥–›7~qu?ãlìÅV?¬EõœiMIXED4FGL J1804.9-1745?èâÎfT%?ýjJ÷uÀ8ñOýnUHÀ:¥}§Ë‹"@© u@t@ë:Æ¥k_?Æׄ¶³…Ô?È#ë†Lá@›´&Ú@š€©•?è°×£Àd	¿Üúû´@å¿è·—{ž¿æÀҝòâ¿ïátYn0_¿ïʓ׸¹UNASNone?Õ¾üô¡–Ø?ÁrÁ"ˆ³m?²›"¨S?¨Eí×Ö¸€?âÞn"Šz? Ón@i@?ف`d'"?ȗ;G¡ Ä?¾íŠm½ÙÑ?´SßIÀØ?ÞÃ<ÿÿmù?ƙ\A
UB?Ô°‹}÷ý}?³µD*c?À)ã*~¦?§Ä&ùӐí?áAvdW»?³Þ$ë2B¼?Ј¦€o?¤|,õw(?»kX9c4>?"UÿÕ§€§?äNA¸ËÒÁ?§ë#wnðz?ʃ[=?¸Ã×÷›?¶N8+Ycã?­®£n">?æ®±¤d?¿&ƒŒçÚo?Åf_òR?ÃAµ6Ù?Å©7_¬}?ÁD¦«®w«?å<%
â˜L?È©K4Ô?Ê~(Nþ•È?«²Dp©R£?ÀZ°G'~A?¦ª"ٔ?åIÉÚvzþ?±ÌMxW-?¹ÙœO<ºW?™šn.Eˆ?Áð֛œl÷?¢ËÀŒ'b,?èH–Ï1Mw?¨\ýË·éOTHER4FGL J1804.9-3001?Øk.Æ«ºGÀ½–ÁxôÀ:NBM'iÒÀ;Äq£±J@š&\`(@
r¡Þ¹?ÒËáÀNå?é¡Xª¼Í@XØ>?õ5ßðëåí?éŸåŽ?Š*©_Ù¿â©}g^ß¿ëY‡ZÒ´m¿ïíVy-?ìÐý³õeUNASNone	?¾³½=ÁÏ?·$íw^¨¤?¶gpŸM®?³·Š¸Ú¨?é\¨/'€?Àt'ãóý?Î'¨þ¯?Ç2Eѵ-¹?Ëi%[aÙ?Åf¤¤ºŠ?á¥ÿÊ?Ãî¾Yӗ?ÖD¶+(Ug?°½¬×搫?ˊ¶¾ü?¬}6ê%aß?Ûõî"GË?±hô¦©¤3?¾-›ÞîŸ?™˜,fxJŽ?áÊöôÇd?­·$Írl¸?ÔÞ«6z'?ªü+›J"ð?ª0TMZ?§ãêq^£5?·sìö]Ì?´*™†‡?ëyl=žy±?¹¸¬·â®?±çÀ."?¶N"1þTÚ?Ñ |«æçð?ÊK.ƒke?äòɨý?ÉN.>àC?Ç.|TºA…?¨*²	–Æo?ÑøV3Ïv‡?µ‡a½Á?á85Ñs$»?¶²»8+¿?˜³ëð͉À?äø–°­?ãÎÝéÞ3/?¶#ët[0M?Ö×lÈ͆?µ‡»2·'MIXED4FGL J1805.1-3618¿é;Ëfß÷¼ÀóÜìՁÀ:wè]À<Rµðè5@VðqB8?üç,å;Xœ?Äôe˜
Ma?çuÜ%/dr@Ÿñ=Å]m?ù·Ÿ•g¿ïøI©ƒò?ïÿߞ¶Žó¿¾í¼[t'¿ã؃ÿÿT4¿ïÿþR€ÖT¿ÞÛ^ºËmUNASNone?¦Y}¬?«"o RĔ?êÃvûc?ÄQ¨‹œMK?¾º]‰sÜ?ÁÀØâA?£M¯ˆÊ?¬íÓñmæÄ?æ"ö°ÝR?Áî[½ÀëB?ÑPpH›?ÀÈdf{µ?ÂÎûµ1is?ªüBòs‰?æ̒†;)2?²Ÿ^ ¸+?Áþº1áñÄ?¨ŽXøŸ[?Ã2ÁžEzÞ?›ÒrÒP1€?å™ý¢W®=?ª	¯õ.Hp?ÆeGØ[Ì/?¢¤BÑ#?–(j·–Ë,?—¸ð•â|x?ëÜli,6?¿LÞçÙ?»'éï>ß?¼Ð¤{RM?"¬8>©?£œ(%t>ý?æ¨\‡ŒÉ?ÈLÎBvOÆ?Ñdƒp@"?Ç»Eo\?±‰ÝÑçDÆ? 94	_Ö?éÇﱏjÓ?®Ùp0U–?ÀROòËS?¨/8*5U?®0"þlfŒ?'–5B`þ?çÌL%P?²–0`H~Å?Êtªe³|Þ?°
 Y\tPSR4FGL J1805.7+3401¿ç69±bÊ6@7ª>iƒQÀ:A8æÑZÑÀ<?¨Ï—'h@p4Æ[D@…6…Î
º?¿m´¹Zª?Ó\K$Á€h@ûd8Š‹@óΆ‹Iö¿Ó˜dMk¿Óɏ*ªÎu¿ç
´¾¹
Ó¿è¬.È—‰¿ïüVB+ô{¿ïÿX°›>UNASNone3FGL J1805.9+3407?昼–ØŽ?ÀUŽ`ð¥?Îސ[NҘ?¿/¹ÖûÐ?ªùü¿Z}¸?œÉ®&£ˆ?æŒË÷ µ?Äÿ7àÓÀ?Ëv¢3F(ƒ?€_õÁL?´¬[á¼ÃÌ?¦u.g,?æÖgËkM×?±›udK¨!?Å8V	ï9?«:LÖ=&?¾ÜÇH?¥
$çÒT?éj둑•ó?˜/
[*?¾¦Çªyá?"Ÿ‰ÊMÿX?¶ÛÉh4	?Ž!'#Ø<?Üþ¼}8(Õ?È;\fL)?Ý6¿ÿ"Ï'?ÄíÃE??·*Kî?©þ¼æ©+ƒ?Þ~JU0*?ɞK­Ûùn?ؽE"Îrƒ?Érë£Z
?Áˆà,Åá?±ùÈöæš?àTÌZ:'?¶PhËùñ§?Òvq
*Ø=?³¡â¤­Å?É¿íÐAe??¬ì!²?à#ñ'1£ð?ª Ü—?Ó4½Ñ 2i?¬Îï_{?ɾùo?¢±!V¯»MIXED4FGL J1806.1-3344?ïÕ
_RåšÀÌ$·omÀ:KX+:@nÀ;©$7í­@*RÁ@|¦CÌ?Ë÷Ám9Í?ºÛ~K››?ôC‰!|QŠ?ü
zW_?ïè³}pn'¿¶1NA+™a¿ê-uïpeÄ¿Üú"[ADC¿ç©E©W|¿¿çh̽]nUNASNone?áÃbr]aý?ÃÙ]Ð{ê?eï ð1¡?ZŒu°b‰9?ÜM\þø\â?ÃØË]¶êb?ä/Û±'f?Á­6ϟåä?‡»@eò?ˆ&?Ú¶oh?Öâp<?ÁG¦ðø®±?åÌWÈzý?²JGæc…?à·‡¸'û?'ã)ÞàE‡?҉Döàx?±'Š5,ðj?ç¯C.ÓÒû?Ÿù³¿óf?¡1"ú~ j?}Ô-×è(…?Ìö'ìò÷?B}êí?Û*™"™³#?Ã<äFÑ÷?vÉ~VüŸÑ?o'ƒà%ÃT?â= 8üî?ÃFøfGv{?Öhá!åÐK?äo,Cç?"BUtâ?™wX»…?ä35\-Rt?ÁÅìÞ»?ÜÉ
	Ó¾Y?µA3rn·?¨óMQ,ór?œ)- Í›?àD¦
?´Ó큼òÔ?ÞĨLKh?¬GÉP'z?¯¥[0ÀÕ?"+Hœì?ÝF¬Ma˜Ý?«¬¤È¨¤MIXED4FGL J1806.2-1347¿ïV'Iµšp@ͨ_/:€À9d
`:Ó;À:¦R©@@P€u[KÖ@<ÿ?æ"&À´½?Ú|ûî"ˆ@Ô²ÄãÊ?@Jîí^Ù?Ý·äx:#¿Ì"è^x±¿ëêQBóH¿éªÞe{…¿éipafø2¿ïãý5Jd¨UNASNone?ُ³Svl?Çsdu9VÓ?ÀÿJ½,_ž?»¾99o?Ýð§Mód!?É7)ëix?ÙÓ+y+?Êë2®m?½áž*¢ëÓ?¼Õ՟"???Þ´mW=Ëà?Çe	Yp	?ÚR‡ó]8?³‰Ú3…?ÆFqfÓ&a?°µ¥±?ڊ@IµðV?³NÄ'E?È5\©àIè?ªÕxÒU¡?½Ö«"
ýU?ªp¿¶²Û¿?æ7Óe-Û?²íÑåßo?ԒP·Iû?ÂïÀÄÎ&?Ê܈›^Y–?ÂEZ•;«?ÝÿjûØ?ÇòRã|¼"?Ä
†õ/Êü?Â<ÁsË?ЂÙä]Ì?ÊÓáåžæò?â»ñPm^[?Èî‡G1—Ó?ÑVc‰':€?¯pj¨îµÑ?Î*3ÎAIª?µAôÈè‡V?ߔ'M «?¶Q=N`?¨.ôø†W?›Uíñ€M}?¾_Ò+9?¾ßÂR\?꫹UÕ'?¿³8ÀՌ~OTHER4FGL J1806.2-2126¿ê†–?›¿Ð)TÂÏóÉÀ7œ;
˜	wÀ9{ÛàfÅ@øùSéa-@¯R¹
x)?¹nV\ƒ?ÔfÏ­QÝB@œýÒ(V@‹Ù_'F—¿ëÀ³ï†59?äɂ—½¿çEfîVŠ¿æ;_ýk¦¿îCC¡•f"¿êÕ!Ð4`ZUNASNone?€9vûÖA?b)Á¬ø?Å3Ñ=Ê»Ð?Ã6§ÇYÆE?êr¾Ê'ÅK?Ãx( Á§¼?›õ)äñU?¦×½ãó&u?ސo)ê›P?ÅWAòz?ß°?#''z?ÅwwPœ.?¸J.äÑ?§œ°'	51?Ù÷SIºDp?¶<H¢q‰¤?ßö'ªúü?¶mj¬¨1e?u*[SNåÎ?a!jˈN£?¾¶Ó*"Ø? ÙVH1Œ?ìtnÅc*?¡`.\íhd?t·ªÄ–ÊÁ?pT8¼pô?Ï^¡moçf?Äoò§ãðf?çþèO#¡?ăÚسœ?""YðŠŒÎ?N잺šå?â]B´84?Ê#"˜ÅM?Ú ×ǸÌ÷?Éîÿ…Ö?®äe(z|Ü?¡\~"PG?ÚTöØËÿ?¹l²<Ëì?àç>@éc?¹E°ÖzŠ0?Vx'q¡0?H1µB?Äc«'»%?°7ûëòw™?êÛÙ&™¿&?°Pe6ßMIXED4FGL J1806.9-2824¿î3,ÖÂÀQ1eәpÀ9×]	ÆR_À;i²lÏ64@ãÂh@>±Ä2ÊX?ɺwàŒGL?Æ"³‰.èK?ÿ9MÿgSÌ?þÒ&"©x4?ïøò?Mé¿â›`
†Ñ@¿éÖJêà¿æá@øÔ2¿æp,XN¿äiUßZ˜þUNASNone?àŠ5În
?¿ÈéîÏ4?…¯jù?{.o2œÁ?ß.6$V?¿Ú¤k5?àô=?.FÃ?Ã8tõ'•?"ôZŠ"
¹?"›¦•é…?ÜØ?Ù×Í?‹ä¶šÔ?äƒã4~s?°¾Áùˆø?Ÿ‰ûœl?‹»sø¹ÿZ?ÕP×$?°p¶&#G†?àžñTË´?¢
ŠÕw?©8N.™íé?'Õò༩£?ۛž§º?¡—‹¢`¹?Ï#Ñv)Òâ?¼ƒÛR‡Èr?'
P˜?ˆž*j:E?çª"Ú0ɳ?½Y§•tŠ°?˃0)F(?¿ófmáô–?žÒT'*–?¢Uè"Ë·?è.uc%áˆ?À:¶¬œM ?ÖËIr˜W?±Ï6€…ü?ª³cåIº?"¸b*Ä.+?ãRd*:ÕÙ?²'Š{uk?̝ÿd¤šT?¡;ÁtšÊ?³qÂÅIç?•êز{kE?æuQîµ)î?£'€ØxKMIXED4FGL J1808.1-1234¿Ým4Á0j@
7S½vÀ9—žþ]h'À; Y}I׺@9 M'Úä@A*¢jùs?Ëub'¬K?à™Ã‹«@çԝ{¦j@Xbz¥c¿ãæ5‰NÈ»¿ÕÉ^BÖiY¿å¸ßDž•'¿é"+Þ«¢¿ïwj·-ÿ¿ïÍî'Ò-UNASNone	?ÉnV'ý!?¾HØóÕ-?Ãßkq4˜?¶…H6¢ì?䬨òýãñ?Â
è
Ó¹?Ê»èvÔü$?½
i÷‰?ÑÉW3ºäå?Àá¨_E?àlZGãÞ%?À¯1ø0äà?ÑÖ«‹'"Š?°›Vc ª?Ã=`%ã"?§*c¢Y	E?âER0¾'²?³@ìßÈÅ/?ÆýÑS¼?›!ï\ýY?ɜ3¡[ôŒ?Ÿ%7O«¢?ãÙ~¹ߛ?£Èƒb™?·—#TGƒ?«aß3¥Ì?À©uÍÀj?µÁ;Æ9?èâ¾!ýðu?»¤%ƅ'X?²ÜD*!+?°-­¬›àä?×f(âçJ?Æ‰Ø?áñc
¢†?ÅËH¾?ÁפŸº£ˆ?¤œeI,…?Ĕ›Å9ì?®÷/] ÿ?ædïæ­H£?³´òÜ(È?ª'ý¤¡"?‰jÿNëz¬?ϒÖ,®?ªD}Wu†
?ær8¥¬B?ªüoNE²OTHER4FGL J1808.2-2028e¿ì¯ÐÉl×*¿ÇN%ýÀŠŸÀ7»èc+HƒÀ9 »åô»ÿ@'p0?@Z"{$c?ŋ-ۅwN?àQµSGP@D¼­šØ^?íå¢^±‰?ïßï¿@P¿àö¨ž[¿àŠN½Ó4Æ¿êd†'UØ¿ð?ïõò`L–UNASNone3FGL J1809.2-2016c?°†ö!—;?Á´™É®ùí?͑ÑCÅ?Ï]ª³¯V?抬í<¨?ÑB1ª>á?¢}îf|@?¬¢Ýÿ¾ÖY?ÞÏe-C?ÊÒ>ŠÄ"?ߪ Ü)È7?ÉÖQ&q?Á9¢°f?ª‰·Êî6?Ô½ñrsð?³5õùI‹?á_øÞ‡?´"Z6Œ–í?^9ªÅŠ¿?QB¿Ø*ˆ?Ä÷«	±?²¡ e¯°?êìå?¤?²ÑÑSÑ*®?©ê¦i›+?Ä'òÏ?Ó^·zŠ?Ðê‹mˤH?äÀe˜,©y?Ò?=¤óŒL?"Eۜß?"Ko"Z?ÞZú£…çÇ?Ð~E'jÝ?àn¦7	?ÏÍhS%–è?¹›àÜ#Vò?¦½m')5?Õ˱u>¬Ÿ?µ =·@"?áæ«)Ü>Ò?¶-¸Gu-«?;@—³æØ·?2ˆ`áŽP?ÆÙ3ЫÃ?»5/n¤ð²?êFW`A¼Á?»@¿Ò'29OTHER4FGL J1808.2-1055?ê•ö–—(@¿ÂÀð À9 Ô ~$ÉÀ;"ËêN½Ó@¸Á'Z@@ÀA¤>?Ò;"ÀÊ5?éXV£zÃë@"XýÈ[@ëLk'?ïÅbu@ý¿jØ»dç؎¿éÍd1Xh¿ìõºAYç}¿ïÿÿÊPË?ïþÍeyUNASNone?ÐZ+öå
l?ÅåŽS"%X?Ò;D
9é?È:ùiýŽz?Ýjûáu?ÉýI'¢m?ق¸ùӍ~?É¢=¢Lñu?͊)•‹Ô?ÀËÁ×GÇa?׸2:S§·?œ¢¶m?Þdu8CñÐ?´çÿ0HÞp?Æ-F+ªË?­ˆËn'€?քç°ÓÇé?³'óYÁvß?ÒDHšß¥ÿ?«mó"Ú?ÑãDRÀAN?¬Â-•1~?ÛØsrùr?°¯ äú?Ä\kT¦:?¿D¥ô_Û?Òá`ހî?É‹‰`'e?áxYzgº?Ê~†®‰°?áÑ:_?¬ú_BJ?Ú¡'þ£<8?ʗ~V®?ÛÚa±‡W?ÉWlÇî/?Ԓøâ÷¨æ?³?Æ`\ý?Éå%›?±"~xð›x?ÞzšŽ%?µs ëÛKd?³wù¯Û"³?™'/&
ð?Ø]|îú/m?¹À‡•Ç8J?ábBR¾qs?¹§fƒ9'`MIXED4FGL J1808.2-3005?º Ïi›`Àd¤L{ÖÀ9âOOÉkïÀ;oÑEØQe@« ¸qÌ@É$¡ŸøX?̀–Rè/?ÑD¼@àÛwŠ{@žªfpwa¿å¶PôåË?ïø曪ëѿ僲ýmÔo¿äØ=‹ü£¿ë©n*¿ïï¢OJÀîUNASNone?×Vl÷WÃi?À;è8Žú?'ê$ÓGZõ?ŸÁýL,º"?ãÅx]glÔ?Àž÷Q…¯?â«msÚ'?ÀÜ*ôÜq—?™Ý›?"¦YZ45?Ù§H{;W?À3Zj¯¡C?ã$KAz|?²x`?«lmÖ6à?–Aj>ÉO¦?Öt)®¶G‹?±Q–[ˋ?åÀ'†ØvÏ?´FšÎ_å?°;æ§?†Š˜þFË?ÐpA•îâ?šú-—¸¤ê?À•ø[NŽ?±:gG÷`U?¢o]†¨?˜<¨‡0&?ê³É±€K?³äOkë9?ÓB2T§?Âð¦ÜO?¦–l;-®?¨Öù@¢¯?äõ€8…¾­?Ã*-cn?ÑM…=…áE?²ozð?¶ñGHœ"Ž? †–ù?ä{x)~Ì?³;‹^ö_?Ü,©usŽ\?§'LE	Î?ºªA¶Èm[?™tû~jÙ?Ý(ÆÇu?§3Pƒ]ê'MIXED4FGL J1808.4-3358?ïÚ;,HTÐÀæØnÁ~»À9…ëOnÓÀ;ÙJr'@pޚՃÖ@Íþu¼D¿?ÀN¢dïBî?éV؉™qV@#4h‡¨ÖM@ð™/¼[;?ïõÞs¾=¾?Èz Ûmé¿àEæÉÎË¿êøToÃÝ:¿ïÿ¥'(^?îK]@ÍЃUNASNone3FGL J1808.3-3357?zvÉ_?F2y"è;?íÞš[Á?±bŽÀw©Û?®ÏT=NR?°lL%Û¥?Ÿ-‡Sš'?¨{£gã9?ç`>ù²Uu?Á#áÖ
,'?΋^i(è?¿¾<ï¨!¥?À¦
ñ/X?§éS»ð7?æB·~½?±Û –ú2*?ÆW} Ü+?«sw?Ù]?¡§‹]Œe8?‡öBs	en?ëÀغ쥅?¡Ö¥½?¹%tyÔ¡:?žaRÿw+?‰3'C1?"€&á(??íÀÛ~~?³Ô8
N]?°"Ì»Ö?²$÷KF=?‹«A¢SØ?—-V+ô?èÙ0ŽEÜ?Ã]$Eß;?Êà‰¶*Q–?ÂÎeÔI?±VQå º<? ÚªèÃÅ´?èÓ+yçˆÌ?°ú?ŒŸð}?Ä)$«t?¬G(»fò?uQ]ZA¬?dêÏ-"}?íÇLҎ?£·ƒ*‰?¶ÛðnL?£:«ÔWüPSR4FGL J1808.4-4521¿ãûØ°¶8À'úƒBØÃÀ:>ýž%ðUÀ;ëø§F*‡@Öáü3í˜@á՚ѧþ?Í»{Ep¢?³š¾‡ºŸ?æ^æªÄdH?ÿ –˜³?³?¡6ÿ½Ý=*¿é†väÝ¿ã@+~³å¿à)¡N™Á¿ïúîéWG¿î?™UNASNone?í0CüÑn¿?°aÂãuøÙ?}ZÙ?w}I¨ÿ¶Ú?´¨2}'º?¯6¿©ª‡?íÁ¥?Óÿ?²_0>X¢¦?rÉ5ƒQ?w?ó"u[Ô?°ÆB¶Ê10?±ÒïÐ?Å~?ìjyæ Þ\?¤nŸ'ʊ­?•vê!"Oª?‹í«®]å¨?·NvA¼3?¢S˜C^)?íšQìˉ›?Œh¬P{N?…)‡›'Ø?d£ßŸãŒ¹?°‹‹jhî?Š•ô³¢œ?ë
œŸÅ°?¹ï@æ¶>&?‰d²6?‡r·†öq?Â3LøEm?¹X/"P?êÑ¿j¹‡K?Ä®/"8D¦?ƒ1;ç­½Ú?©¨¾!N´?Åî"Ñ;z?ÄWñιáä?èe.i¹›Ü?³Ã|3Z´ý?¥±ð.å?•†2®?É#Zx—–?²K̯?êjêdÖ?£†¬[WŠ?•Ï'æý›?Š"y\o?Úræ3õ?¢­¼IôuAGN4FGL J1808.4-3522?Ï$][¿ˆ/À•–\Î70À:ôj{žÜÏÀ<aÏ'ðà@@W¸"Ç?ú«»Š…) ?Òt¡ýì)‰?èÓ €étx@
†ݒî@g*÷O'I?ïù'áê@P¿íßRáNd?ÝÊ®›¤6¿æÄ}ÈØ¡¿ì•à<Z¿Ö×¹ºÌD<UNASNone3FGL J1808.4-3519?ßg÷"¨q?ÊúãfþM	?² /ÎKhc?¬D^'+
×?Ûïüxr=Æ?ÈöÞ2½;?䱤°×d?Æ¥?<øÚ?œMØ°BÃî? ÈY8Æê?Ô×Ùñ¾8?ÅQS±Ð>"?é'<!•/?¬§^êvIì?°}àYO¬?5ƒ^].?Á¸²‰ð?§zÎ{;?ìˆ9ì,è?•ÞSæd¬?—'§¯?~èýr£?µýX†‡w?"!dԕîê?ÔîOYl?Ƭð%8ëü?¶Aâ
	Á?°QOޓ?âÀœ:¼G!?ÇÔªw(?Ûò–†rS?Í'/hg6_?¨!«rc?°rȔ@Úµ?à}ý™žL1?Ì4z'…ÍV?äyœÈtN?µÛ6.%²`?»®|YÄ?¦¬8hm‹?Ð ÕÂ-¦E?³ "ËÙ§?èEýE©–?®B&D|¥?¢nˆNç›e?'jW/é\
?ÊLh×b…?­F-Š'MIXED4FGL J1808.5-3701¿î!hÁ›§wÀ \¥ß"9çÀ:%а‡éÀ<Ö¿•@raÆn@«ñ'l?Äær$àŠ?ÞÿÛlø§@'c/@ñÑHÝi}?難¥¦V¿´'¸N»yé¿âÁ' ÿT	¿çaÃ3ÆÖê¿êYè©¢%Y¿ïþÏ´ÙéUNASNone3FGL J1808.4-3703?ËBˆ¡àÌ?äÞå0Ï^?ڑ8\<ìÅ?Ä:äÇ.A ?×ä¦_r"Õ?Á¢®åŸñ;?ÖÑv†*b:?Ç/{ eXÓ?ÅÔ7­ÉÚÞ?½Êó%H†N?ÞDm¢ð°W?ÅöœËäV?ݱ¶óéé‹?³NàŠ@?ÓW¡£9'­?²0ÒruŠ¾?ÍíNѹ	?®Y|ö…3Ú?áaÒöæˆ?£XBÝÜOÞ?Í1MÂx'?¡8G› ?ÍGfaïðO?žEÿÑwz?³õ"æ-PX?¾ÿàdHá?ß­¼» –½?ƌ
Š,>L?ÛTÞ¬?Å
镸ìú?ÆfȖ²3™?ÂLÚ%rLÆ?ÐëO´>®?Æ4¶¯ÃÁO?áð¦OySÃ?ÉÊΛÊÝ?Ï/M= t?±	‹žHâ?ÜùJ¤ÓÎ?·õ¿<ô"?Óo'Ѽ[ø?³®£Z9g?ÌùÕþh•?¢¥Õüœ)^?ٙ¯©{cù?° ¼a?×éeWPQ…?ªŠJ"#3ãMIXED4FGL J1809.0-2853¿ë¤•µx66À­Š—ž×À:]xFÜ]À;އ$L£@v ís`@è«ÕÜ@?ÒíýÐ?梐MÀ}3@ÃèPïÝ@%&¹Óø?î)<7B·¿Ô€ûþh¦2¿à°ž~蝿æ¢CŒFÊÀ¿ïÿÿ)@k*?ìôí²öaòUNASNone	?Á¼Wߏó?´ÅŒÆà???ԃ§Évð¼?Ç܉Ý}¸×?á}=L£¥?È95ʒ5?Ø;¿i!?Æ:‰¢ÅV%?·‹#«0
ó?´ñuÜ?àð»Õê¾á?ÊJµõ‰ž?×82·ô^È?±?@Nýÿ?Ѕº*Äá?®ä"vã/f?ØBʍàÜW?±¥)IQš?ڊÔ¿+ò?ª¤XaÜb?É=i0ßà•?¤D»:¼!?Ø×/'ÐãÄ?«3'ëC"Ü?²­'w
?«" ûÎó?Õ§äNžŸ?Éïv°`…|?âÖÅÞéQ_?ÊΡ
VU?¾c,`2x?¹û WҜ?ÁÁ¾ˆ³º¤?Àëkãü?çÃ*ۇ?Ãc)‡°/€?Éfœ:Íu-?ª
½ÑÞäº?Öûâj	?·Ôí8ÅG?ÜPÏx:`?¶t8찗ã? ÅTTã?¡9èÚύÕ?ÐË\5q76?²¬*¦RØ?ã)³òO,?³Ùé?&ŠMIXED4FGL J1809.2-2726¿çMÖªœ ]ÀÞ9ܚ À9"©³`ëÀ;32¯È@ÕÜÔVÙÖ@w¶ :‹?ЛB;8æ&?Ê扷N``@
Y*f—@MŒ£ ?ïûÏ^¢wº¿ÙEíÊ»{¿è"d~.Ú¿ä-œ»	h¿ås°Á©X)¿ïÿýawUNASNone3FGL J1809.2-2725?æMÐ<KŠ?À%z¡9~¯?˜Ž\_ã{¡?¤<'i©?ÑÛyÁj¡'?¾çÄRˆk§?ÞIÄù³yƒ?Ä¥ôwFï?Ÿx{­Cœ?šoíË5x&?ßÅS6Ÿ'?ÃÔZ;F
g?ãô÷gk™?°™…WÛB¸?¯À…"u=?šwjlEÔ?Ôa]F?¯ÓÛB?Øh>1,â{?£6µt›§I?±2÷®Š³?‹\Êr/È?ᥞ¨ª·,?¢ö¤Î¶Cå?ÚÉÄo09"?Ä.C»§Ç–?¦^œr°Ú?Ÿ%æ`˝?á9—Þ®v ?ÄWßM`Ž"?Ç.h_Ý,¹?¿Š]ôI_è?ªAÔö?¬;Å0©Ê?èT*Æõj?ÀjÄL©?ÖÉ}%ßQy?±	 mT^?¹Ñ*ø?¡w-ÿ"¿?áwïk:ê?±É´oï¹?–êÄӈ?›i²ÃƒšK?´¦U?§©µ?›`@BÌj?èÅz¦—âh?¡TLÂØ*šMIXED4FGL J1809.5-0816¿Ô·YÌ,Çg@¥ÊÞ¶]À9gÙÛ©¢À:ì™+µ@Ꮐ[@ôØý\·'?×T=ø´?âÙ`.@÷ñ"íjÒ?úe–w¦)Ë¿·ZŒhƒ¢?ß:…\ '¿êž`lQb¿ëÜÅ}Î¿æÈ|`x»©?ÈäD˜`_UNASNone?åðÂ@4?Ƥ§C@™?šÒ\Á'€"?—£A
;|Ù?ÒqU´"Ã
?Æ>ƒú?٣ޘŒç?ǀ'ˆ>Ž—?ǘCá´Ãõ?ÀŠz,kî¼?ڏÿx+ñÝ?ÃÃïK?Üs¢£?´¿}Å,äG?Ã{,7&Ãõ?®>
‡Ûež?ÙÏLBgb?´CÌy{þ?Ï\Rˆ°_¦?¥¿{œ×²F?Ëü‰?§«‡Ÿ¼¶?á-.èô?«ӝ"1i?ݍ…Ø$Ln?ÅÀ7h!&–?±Ã ºÉ_È?­ò:@y?Þ'ùD؀?Æî9Œœ8¹?ÁÑÞ5>M?ÀÊU°ý±?Ö=Q˜ÅÖ?ÉOÑU÷è?àlߦ»'?È&"Ql6è?Òԅž¿ì?±«¤©°!¢?È:ŸÛt}?²Ð.ÕK8?àuîÍ0RŒ?·ʜf–?±àŠ|—Á'?•èÜ·±?ÑCýyŠR?¶ÎqæÂÚ??å"a±Ë¿‡?¶CܟÑâ£MIXED4FGL J1809.8-2408c?ê×<$H‰²ÀDÍt'yÀ9$«Ô.ÁÀ:{Åyò4e@;€3ìì@>üå™Lm?Ñë>|è]ø?ã¤WB‡'@d>mùÙ?ýƒåîy¿ÛO[²Ù1¿à¾Ûrþ¿çŸTžè¸ç¿ëXÚϐ¿ïô…¾Eu€¿ïüø^KòUNASNone8?ÅäŒÇy%Ü?º:Âð;M?ÒaÙluþ?ÅQE'st0?áz+ák{Š?ǻ嫸L…?ƁÔFúÌv?ÁØð²I'?É.X-³?¿ÚýÎ2º?äX66?ÁzýУO?Ïz/Œñ¦²?±IþÂ6r?À€RF…Ê?¦iì°Í?ä_‹"Tá?²¤à]Õ?¡…NÁ«œ×?€•+q°û?Ë£ºË©Y?¦`êµò¾ð?çþ¼`Ãå?§@~ó–‰F?º"øRŒ•?±BÝÞ?ÍŽ?j?†¥‹Ì?åiØ¥ìÓ?Åä¨Ð]ñ?ªÄ·õ7?«?°† Žº?Ξ-ßّN?ĸÕûZåæ?æ¬)Œìb?Ä@‹ãðÍ?Ãý½‡y?©­ˆô¹Y?щ»~?¬U˜©RËß?æ[Œ²oB?³*EP—?€#æ#áâ®?f"¬Ð.?ÏVxI_;ò?°°Õ<H_ß?çéÒU+Y?°¹RˆUROTHER4FGL J1810.2-3054?âšÝ[1ÌMÀfù3]$žÀ:{ç¨ñ%rÀ<	0pá¬@g0{óÁX@D'¾‹Áj?Òٛ\'R(?ë¬<Ԝ¤ç@Ñ÷ÿ€~@@ŽFø7	?ï÷`‰­"L¿á1;A®A¿µù3¡ÜÍæ¿îÇ[¾í'¿¶",maZ¿ïÿѧ' ÖUNASNone?ØhTûÛ?Æô­ÉHÖ*?¯kJñ}Ì®?¬T}­@D³?áÕ>Fiø?Çm[?E?áæ	%\tº?Çô䔥Ð?¡]¿§4Ï?¡¼4nߖ/?Ú5ÀΉ2?Æ@?=á¶?ä*Án†?±VÁ¢Š¡?Àêjyy?§?nvr{‡?Îm¦­e?­ Ï°]ó?æf:x¤A?¬ÎïM?®˜YVø#,?›œ—u³þx?ÎÀÿÉFî?¨tNc=ј?Íivç#K?Â6¡§°Å?ºÁŽ}©?¶Š(׫?åMxoí«?Å:q9—ë?Ñp-H§R"?È^L¦÷¦?³NæßEëà?¶v{ÖþR?äÞ€â?ÈL@?¶#h?Ý<v±jÏ?²Ä¤íßÜ?ɸ©ez¿J?°À4Jãê?Ön֑5Œ?±wÑ}ò°?؜Œû?¶ƒ´¦3‡¡?½q=s´4?±‹üm¼U?à'	
n?·|ԉ¿ïMIXED4FGL J1810.3+1332¿ï`_4ݜ@.A•övêÀ:eÜyhÀ<¤~Ïé¸@iÑãâèî@k;¸<òÐ?È÷èÔë?Éٕ2+Ì7?ÿ¡Ž«)?ù½X›L¢? Õ`¿â4Šˆ×¿âÚìJ@•ò¿æ¦]—ŠË ¿ì¬…dXo-¿ïÿø¨ó©°UNASNone?ꪪþÆÄö?³²Ånòl"?žÅ0ü@:ª?'¦N ™?Á|­æÒ?±êùuCÆK?êuáõRþ?¿³e#ßó?±µ¾³h?®1PʑÁÛ?º¢o3È&?¸þqpÁÅC?ì–AÚã2a?¢ËvnBê?£D¹®½G?•³€ï€`K?±«"OÐU?›W¤½1:?æêžôLm?pN"¡
i?·zy;"Ñj?Q/ãìzÇ?ȘGs'X?—ý@ìR{?âΊµƒ¸?Á`Äx+?·v̵Á<?²Š38…?ԅhâ9?ÀÃ[®?ã©ë¸#?É!Þ4†Íî?Å
SCN?Àö­hOìõ?ÌNž¶d?Ä6'Þa?è‡GÜQhí?°y˜žýµ?¶U™~Ȇ7?¤âH"Qâ?¸ύð?§FØ
•b?ܳaô3:Œ?¦éòô0?Ä®(+,Ú?¢""»s·?Øõ‰öI¯?§:¹¯ ¯òAGN4FGL J1810.4+1700?ïñî…ëM'@0ŽÓǒÑ(À:l0 ±»ÏÀ;ÇVpOu@™¾JÓãÂ@Þ?©c;?Ñ8š{@èþ?ÒþÄt¹@b¼ºh?ú[oó¯¿ï¢36ÌE?ç†tX—pÊ¿äÜþޗÐl¿éÌ«ßí;¿ï°ÿ笿ï^­À1ËUNASNone?ëS|£Xy?¼CKìZ˜?'ql*ªá[?ŒpÏ×áV[?ÀƒßëYø?»ÆCpÃ?ê `…{Õc?½õºÏÊ?¹PïyӉ2?¶Lu­¸#?±¬YßØ3?©'=bŠYx?ç´ZBÊ3?¯i"ïû?°=då\ç?œ(1•m?ËYä'(Â?¬_–W¡Ù?䨁¥bX?¢`T\+W¥?ÀÎ^=ˆ?›""GR	?̏á
e]?ž4mÄ
?恢pǂ$?Âö	øÒ9?§Ûrq«v¸?¡R¼ìS&£?ÐLÐW	Á?¶Lá,?äZý¸¹+?ɊæÙ€`?Î,ÎÓjÔ=?Nj-ۅwN?Á]Å5²G?³ñùu—ô¸?âSMN+Jö?²ÆhÈíúW?ºäæã¾Å?¢yhPPÅ?Ô +ª¹ã¢?±`©ôÑ;?ٌx‹ygÂ?¬IÏà[(?ÉēÃ@Üê?¯>´"Œ'?ّ='æ)É?®×Þ¼£ÝMIXED4FGL J1810.5-1415¿ïÎTgÇu±@·|ˆçš®À9(ê°£À:ˆ¿™Þb÷@ÕÒmrÊ@ìbÿ©˜ë?ÐÁ˜ÜZ^p?Íîryo,´?üQ*"ÿ&?ñ?ƒxšñ]?ïb´•žbV¿çWy-éGW¿ë:§0[Ÿ¿å+,Ôt`û¿ïÿü¿ÙŸC?ïÿÊjåQUNASNone?àïÔ/'ñó?Êä²ìG?ÇÖ(Ú?œ•,L%?ҟl®.?ÇFz…#¸8?Öiÿæ³0w?Ír¸?ˆ<`?»ãX2#Ç8?¸…²Ç¬Á?áN•aîÝ?ÌKy•å|?×»ÔSÌ'X?±õ$ãAáÕ?ƘƒSüd?­
dÑɈ?Ü÷ê£Úv?³Eª²ó<5?¶‹Õ/Σ?š·ÏˆÀ·?·g¿º$/ˆ?™^ý†?êAb˜j^?¤ãպ͔õ?Ùõ‰²'–?Ɍץ>?Ò(j[h†?È#³ŸdÎ?Óâfòoã?Ë#?ŬŒ?À}ÆهŠ?Àç)¬ï?ÇQXÀ¿?Ç,(¡x¤ñ?æùómí¼?ÉéBTÊmÞ?ÑgSÓx?¯ƒ21Ò÷8?ˀ‹7£|¿?°˜¿8²r?àš)°cƵ?´!Ò*O?"T^½TÓ¥?\yh¢?»áéÐ¥?¥ºMøé?ëûù­wê??§ÜÃZ DMIXED4FGL J1810.8-3347?î'm¿²CÀVAb ßÀ:<piõg À;¾9ìN@ád^y]@|ªu‰ð?ςe"oä?Íöc7‡×@œd…D@³jÑ?¿¸v×LØuÍ?îx`äÇ?¿äxrØd°"¿á,|Ë,¹œ¿ãúÍ[h£¿ïü½Í«oUNASNone?çpµU?¼ÊhwhÑ?€'Óƒsˆ%?q•Ø0¾ô?К¹$ß?¼¬CTéfa?é
{é…j?½°%Ùû«Õ?9i·?ŽÃéêÛ?Êè9Ē?¼PÏ\=?èÈqÜa¢?«gÌmÒ"?ŸÐ]Õ,Ê?º.›'?Èä7ÄߺÞ?©Dª­R?êô[à.1?"5ž4˜ií?˜þJÎNdä?v&0QùR?ÁÇ%{j?'éTøå?àí¨ÄÀt?Ážã¿q^V?"J®
¿½7?†bN-ˆÅ?Üð––¥?Áši£1ÈÐ?áß; ´ÍÊ?ȟ{×xµ?"o(hD'?œ´óãܓ?Úú—7‹ÿÊ?ÈEûHˆÙ?á]¡H×?³]GGõà?¯GÇd. ?š
ùíá'I?Ù[čtX~?²‡½âÃ|?åàa¶Ë¦?¨@vé&±?¤îôOSÂx?Œg~¥ˆ¡`?Ñ¡²Œs…?§¤.­naAGN4FGL J1811.0-2725¿âSŠIM/Àh"!'÷¿À9ëˆêá‹À;ZÆü©3k@Þ´\"~Í@vœ©ïR3?Ïx´‡0¶V?;:bÒ]@rpŽ@*;±±éG?ïّG=V¿¦©aD¿¦SÛÓ¥Ú¿ëˆÎ™«¿ÖЀáf⸿äoTˆ'UNASNone?ái'?Þ?Éô‹Ñ;?ÿò€ö½?v?cµ·}t?Üq-Gi~§?Út­Ho}?âf¹;º/*?Ã=?n³oŒ?ŽH–Ñûü3?'¬_óDU¦?Ú@HÑ;W«?ÂsÎ+¾í?ãrGßMéÿ?±o\YGD?¢­0z,À?'ÙiÃ\?ÖÅÊ>ýìª?°ÀM—ËSÊ?ã'JÒꦰ?§ç_V9¹?˜*ªn?ç?ïѤÄæ:?Ø.¿²QÂ?§G…¿1#?э€"Çw›?¾ùRñ®?"*™öO–Û?ˆpû8òš$?æŸëéÇ|?¿Ãúš6†?ÑØú+™zª?ÂvHå)Ã?–Íêµê(?Ö·hõR?æc|{?Á¹¦aJ•?Ô~Æ)q¾?±M¡dp±?¯\ž
2Ò?—@9sAªÀ?ãÊÓa+"?±Õ†*-Œ?Ó&ÔÖ?¬Mä…^?¡×°¹Bl¼?"ªׅòÐ?åY~àÊtr?­Ur0ö¢FMIXED4FGL J1811.7-1442¿íêE2º?þ	üD}ÞÀ9ÖÄÍ$À:ÿöÅĚÏ@ŽEµì¶w@Ã%Nn"?ÐýGþœ?Ùp ¤eP@è%@+i:?öcˆm¢Dä?ꐦv î?Àá®Ú÷³¿ÚڞÜúlm¿ä½ì)‰fF¿ì?韖]пïôÞcβUNASNone?¡l"çÒ8?ŸÐŽ8ˆ3?—¹g.&G×?—l%[óà?î+s=[Í~?¦-'Æç‡C?Ѡ܁Ô3§?ËoY
Q; ?½ B.'~a?µü7š?㋉yÍÀ?Ê@»Å/A?ÎÐEûëPú?¯¬ßËÆ×.?ÁßEº
FS?©}`ê*ʒ?ãԁÚ-?²Dn[1¼×?ºP9~âð?Àç&ÅZ ?·T\9?˜˜L)³´v?éÒó
d}¿?¨¥oE5©?˜ûÜeä8ä?ì÷%,E?¢=´CÅ?ž–ÔüD?îEÕ!Z?£*¸òA©Ø?ºVÁ²\‹?ÀdÍVä?Ãb÷WK&«?Áƒ½æQ?çÜiócºe?Æær¹
°Ë?ÀÄN{?¢ê}`ù¡?À`¿ÕºÔ?ª×¤¡rq†?箔0+Êg?°¢¹y,?£j‹ÛY?ìoÅÙÀ0?¶7$­ª	ä?¢|Ù9T¥î?ìr±"wN?¨pÌÒÉ>ŒOTHER4FGL J1811.9-2336?҅8eÄw`À¬|•|ÔgÀ9\Úx†ú[À:¡?´‰	@ð"댫u@e€éŸk?ӓI]ìð.?áK.g˜@Ê÷	·8ç@g|"¤b ¿ØÏ[†I¿Üw†´º‡P¿è7¾³.–¿ç©ÇÁJ¿ïÿûÎBÓ?ïCÿ3QfUNASNone?Ò©£?pê?ÂÑå4——?ËÆaÃêP?Ä>Dštò?ßs°zËg?Ƃ¤fŠŽ?ÚÚàÌ3æ?ÉÁzx?¯RK¦?©é\wë˜?à¢~5Âr?ƶ"
7Ã]?ؘK¡û#?´"'R†?À[%,VÂ|?¦ùÛ*ŒV?ßËÕÂà?´òšå±?ÄPKiWSñ?¥ŠeÍxê?´ûYõa8?•í÷%?è[­º°7?©kàh~ý3?ÈîtõåA?»oÝLe£?Ǎ@Ýb=¯?Ä>…àîå?ãáŠØFå?ÅàÈö1'É?ÀSÊ?½G¶ÍÜí+?»;•
jr?¹ê£'-ÿ?èu8l5»×?Á«"Eõœ?ÈAIEw?ªñtÈV?ÂLŠ®Ä?¨õà6IÌ?å\š¬'ï"?²[W‹µI?£1(ЅsZ?¯ê÷Â"?·¦øô­m?¢Ï˜!y6?ëØ+ôNl?¥m	NÐvOTHER4FGL J1812.2-0856¿®³xp‡°@ãâ"À9iÀv}4ßÀ;…nij'@I†¶º'@{©f–7?Ñ3a×5†?éU—¬Y¾@Ót62Áô?üq˜ç%á?ïðdìé¢Æ¿ÕUÕõjzÈ¿é®Æ¼èS;¿ïÿ–Aö¿è»À½Iø¿îQ9]ïŸ`UNASNone?»÷ªl¶È»?¾µE¾óg¹?Á‹Hé'÷@?Ã¥b´™éå?è8x)?ÈÀ!ë?ÆÖ~$PÊÑ?Ē,à*D?ÙDC½UFÀ?ʦfÖ³Ë?ÛP}0'SØ?Äqµ±ÊŠJ?ؽҊD?´}<Z"
?È®«þºÊ[?±ß°×EC#?Úê×v–V»?´7ÊP(ˆ÷?©:
̒†?"Ø«y×6§?ÛZÈvY.?°Ò¬î\«?à¾úóaó ?¯
(a½?µ¼º\OÆ?ºóióÓe²?ÁŠØ£<'?ÁƒóÙÅÈ?è岋ÐO±?ÄÙíÃM®E?¯whòP͟?¶òÍÇþÅ?àÙInI?ÎHÌöEõ‹?Ü`NkÀ:?Êý+]ë‡g?Ò:fI¾™?±ñ=ït£ˆ?ʍÖ́¨Œ?³ì˸k:?à?ˆz¶'?¶·ª.oÞ?…h÷¯1Wý?l}!?ÞVH_•<?¹–N®ç~?à}±'?¹Nˆ5ÇvÇMIXED4FGL J1812.4+4441¿ï­3ğùý@9TgÓMðÀ;N'™ð×nÀ<Ž˜÷³*d@yòŽÖr@ ؽ›×a?ÇbY&D¿š+WÅ®K?Ó4ý¾1@ÊæÞpä¿å#ãŸw),¿Ý$	_$RÆ¿èr¦äÌÉ¿ÑÀWs"\¿è™\þØ<¿ÔðáxÚUNASNone?ï°÷³øŒæ?ŒBíK®]?WRÔ²ˆ?aˆû0[`?€×Ðï@Ê?‹®Û—GH?ï¡Eo<?€ã´ä€‹?\€N"­‹?`‰Ìeªnö?"¶¸!X?|èJ]ò{"?ï0H»ÁÈÉ?Š4n:¨ð?j±%{¶kú?oHÂHÝß?– ÃÕ8sg?ˆ ÇzòGW?ïg%í¿$‡?pŸ…²­?`›ðÅP/Ü?EË;èPá³?'Ä6Ԓ?p@0ÉUÜÇ?ïV¨þ/ñ?±|ì
$™?e¡M)jèÅ?_gÕ½éZy?'vĘÐåÄ?Ðè`27
?ïšµ‰ c?™VÈѤÿ¨?i¤[?t¤‰¸¬(š?škè¸9©?—µ"d[Ó?îl;í8tˆ?•"ЬÖ7Z?u€ø?ŧ?u"T^DºŠ?¦ŒAº™I?"~)`Ø?íà4{»?å?'"¦‹\¤x?|úè
Lô?jaÝIn¡?®][Fiõ&?'<‰[#‹LAGN4FGL J1812.8-3144?ìj¨>ðM'Àýœk1˜À:'È-*ÛvÀ<0æl±C@Ž!AÄ¢?þ_æðd'?Æz>ŠJc?à·l³‡i@þ•`Nõ1@')ó?ïÿæj,Ą¿ãšÀá?µ¿Äx@Ùd	ë¿ã,æ³'à¿í…·š5 Ì¿íؾópPUNASNone?Л–ú-B?½óEz'T?ÕÔ¶â;?Ãær²œlT?Ú]"Nðº?Â#˜ÝXó?;{ãeý?ÂT}ë´?Ñ¿'éÌ.d?ÁÛ½"T?ßa?•Âž?Ä~
!%¿'?ÏDEÁ͌³?¯:]ÿý‹7?à±{´<™J?´Ðí-jqc?ÍõËm@'?®€¸øߙ;?áç˜Ã/êÿ?¢WÇ³›>?˯ÜÓ? yD…-5t?̲'ãc€ó?œDD'¢0l?»[n{2Ñ9?¬p⚃=Q?Ù¿â4#Y]?Å£ë;;¯?ßiB-òU?ÄG+çÔ(û?¼¢/¢&}e?ºéÑ6á5?×74$î-?Èߊtb¨l?àÐú5)œ?Éé¹þ¥B?ÀÖÔ$Q?¨¾Fóº	?äT›…¬ý¥?·¨­Õ-?Í×vÒwå?²`K¦8ç½?Ô t °œ?¦{*iqCö?ÓñÞ¡E¾?®Ôr2"«?×í­Í®6?ªô"°qMIXED4FGL J1813.1-1611¿´¸÷òò#¿?ë@dïmâÀ9.ð®SeÀ:J£Üºî@øÓ4ð͈@i:Áœíâ?ͳðÈT˜?ÀVT_þ˜L?õ-ŽxÔ'4?Ø٘,‡"¿ë³Na	y?ï2a|ÚQ¿æÙþäw
~¿äHîៗµ¿ë¨a}ÉY{¿ï¹úݬCUNASNone?·¨V@!°?ºrßa§v?™ŒÞ,'Y?­)C¢ˆ?ì>—"¸ÙG?½Ô..ÖF?³òVöN(í?¹SÜ×ùÿõ?¿:~£kvé?¸Qªhï?éšeLòU?À_¡Rm­?á"KT?¨¶Ñ@"?ÁQéȗD;?ª ¨@KU±?æà z©?±^MǨ?£îþ§š¡?
=fU?·xl¾PO|?Ÿ2c#ª™?ëßÃxK|f?¤÷ÿ{VÕ¨?°M¨àv‡M?´LÉ@Ø
¹?"é=yeÐ?™d°g'?íW÷ïÖ?µ×ÀðXiº?¤šT÷Ëu?«d}ò§­?ĝysŅÂ?Ä%2ùkU'?éŽüS'ç7?ÄÐéãwÎ?¾ûÇ¥à=²?¤(êvÉ?ÁNi> æÄ?¬eq‹íæ?çÌì»»¾™?±Œ ýT?}2ȹž›?€……•Ÿ?¸	{ÿ†²?¦^ˆsþ?ì€êe†cÿ?¨Ø "qZeOTHER4FGL J1813.2-1128?ì&E9£˜T@Ȑã²°À9.@q	W˜À:¡»á¸@‹Ò@MM@SÝͦ?ÆðtöL?Ò}PbÃï"@ÇÅ&^?éÒ°;¾ê?ïO+.?®¿á<W3Ã{ë¿æÉvÁ}cX¿æORîº]^¿ë€uf¿ï³Ñ¾¤UNASNone?¿®qú»"ã?¼wñmþ?Æøá2ŠkÔ?¿1¢(M?é?æKùtòo?ÅpC-•ÿ?Ça$ÙºW;?垈'£?ÑoÚ•\?ÆȆI¹:?áŸ~ܐ"?Ÿi#Á6}?ÍÛÿ÷åÄ?®ß¥ÐY€?Åë«ZóQØ?«‹…SÃIâ?ã+'²?²—ùOo{y?Ù˜¬›c?2pzq?Ȑè®]S¡?£œURñ(G?èìùué¼?¥dóë6Ô¯?µ³âÒêëh?¶ j³Y¢?ħðÝ«ÊÒ?¾ÚÙÚN‹?è‡n7¯Þ?Ã¥=~]?¬¥o¶}GW?µ9AYm'Û?Ô ¦
7´?ʄ096`?ä,±Ê	p?ÉÄJ/¬ž?ÁeÜgØ?¥CìŒ,_	?Æ t–?«D¿_—c`?æžßÙD?°ìšBÚòµ?€Dõ"OP7?iBå¸á?Ë$ùùD"È?¬2¡·Ò'?èõ­«–¾•?¬Ú"«[("OTHER4FGL J1813.5+2819?Ыˆ±ŒKö@41ÿ?àHÀ:Ý\úŽ§À<­½MÓÈj@Püi¤&?ûޑÖV¹J?ÌðÔ¾Þ¢?àM´ôhó	@jÝÄkÕ?ôÐÓÇè·d?îßÛgšC
¿ãç- I¡Š¿Á瘋§"¿Ü«´NPÅë¿êtÝAäüÄ¿æPazChUNASNone3FGL J1813.6+2820?ç+ûÎíäJ?ÀÁ8=ç ?Ç`'+"׎?¼'Öå]?·ß/Cm?¬@C'w1H?àat¤—¤w?Î4Yþ Á?ÖÙ˜Ì×?ËU™=íæ?ÀÈ<	4v?¸Dà"G(?ãƉɏM?´b
Σ%Y?з'óºÍF?²ê·½ü?¾í¥èåå«?¥ÍT‡?ã!îî›åµ?¢oc¢'6ð?Ì<ü¸?¡~²ƒ7'î?Çl5rls?—7ðͬˆ?âšX½²…?Áð"Â2?ÐtÛ¿XðÝ?À–ö7\ì?ĬåŒóT1?³¢O‰ãÀ›?ѹßPCJ"?ʓh¬U¢¹?á‰Œ¼w¦?Ï==NÀ?Æh,‡Œ@?Àœ1Eê'?àP¯¼µlM?¸ÁŒÞ½i?Ö	HLù?¸Žu¿˜Þh?ª¯ìlO_?¨÷l¦¤ø{?֗¬5Ów?¨²/±>?Ó¸c+Ñó†?°|²Fþ[?Õ°'ø9?©]0W—³¿MIXED4FGL J1813.7-1152?æã"î^íÌ@IÅÓï×À8—¡Vý<×À:I">¿@0êp ÏX@3¾sm¶?ÆZ"Zî
9?ÆkúdŠ™!@D,Ý®œ`?ø9€=Òô¿ë@tdUë?ï^µÍ¬Æ¿åßÁ œ,Ç¿è½^®(¿æ˜~±¶ÆÑ¿ï÷ýO0ÀUNASNone3FGL J1813.6-1148?¶aÇÁX?¬4DC:&?–©YJâ
þ?"÷*MÄI•?ì~|=¤a…?¯ã¼Q¥E<?Ã
…N³í-?¿ÉIÜ(E«?аW Êý?Æjéê?âärÛ¿®×?Çö57* ?Ũ­ñóÖZ?¬ïr}ƶP?Áp"Ä´'?ª+ý´*ü?æ9³RR]E?±íAqd?±Þ Jª÷z?iy¥º7•?ÂY€Ç2&?Ÿ	ËÿÊ?é?•–¢×?¡ölªu?ªBg¥øïã?ž+'>¬D3?–¥›¯S)?'÷Š¾ôí´?í¦¬¬ñ»?¤€"/lX?¬C`'*í?¯!1.o?ÖÐ#:äû?ÌeäQ^þy?ã1aëòÔ?ËK"ãªý?À3f‰ÌÈ?¥-ÕÆޅ¹?ÁM¦|,?«"'xn:k?ç¼ß¼¾ŒÃ?°é""?˜QpèVî?‹c"·oÐ?Å&!êWïx?¨Î¼ƒVö­?éóìCÇ«?©D€F8'øOTHER4FGL J1813.7-6846?ÙT5SkYbÀ5Üك"t—À:ÂÀ<G³"ÛÈ@ȪWVþê@çLû‹&?Á.,¹•?ÉvÙ%J½>@]o¿«|@æW¢Ô*å?ï'È#ð ¿à€Õú¿ßìÐÃ|l¿æÜN_‰}m¿ë&ojñæb¿ïÿö$´ë/UNASNone3FGL J1813.6-6845?íŊ[Á¥Z?Ÿyªp>qú?™'fñçé}?f¸ì|1Ø?¦Þ&Ï=8œ?•ÌÊ÷Ê!X?í³YJÁg?¤³žô"Ÿ? ã$@ëÇ?™)û
©¥?¤²×HÊËË?›ó¥wÊò?ìŠÀ…80?£í<'$fz?©	$³;÷À?›b.¸*?®JÒùA÷?™G£zˆ?ë'8óZ?ŸWö@vƒ?¯ºaû|ì?"{©§UZU?³™3ŽG¸?ˆÑz$—
´?éõ]ֆG?´"³×Çø^?¶IÝÿ$?ªëÞS¥?º3Ob¾¼?¨Å-6¾æ?ê[6¢1?¸ä)9'Ž?µ‹Q(!îN?²WVë(•f?º9Õ'©.?¯ª¨k¶µÉ?éc² Œä?°Qò0̋?¸ÐVzž?§š<Àp`?¼æ¨&`?¤[¸ç¬eé?åØÉ"a?¢Ï1/f¹·?ÁŠ7,x?=?œVúb²&Ù?Ç©®ÿK>? 
©µìA¤AGN4FGL J1814.2-1012?ç™÷_>÷.@ÑăR/xÀ9u]ù°Z¦À;§ž?È@†ò¯	˜Z@$Øý\·'?ÓãҢϣA?ïÎÿ!]ȳ@v9þ(k?ÿü¢¯»Å?í½Aߞ`©?·ÔÂ]³¿íw6,â·¿å³:Š?‰ƒ¿æ4á‰t¿ïÿèîkƒUNASNone?Äžüð?¿©´ü˜äµ?ÁsãßZet?¾»|$`)?梟I(_g?ÆSŸÜ¡#?ÒXÔÏÇö?ΛôaUY?Õàéô>Å|?ɓr/s?ؽ6ñr?Çڙ
Ÿã'?Øt Ësþ¢?³aË1¹ƒ?È_׃+t?²&ÉÞÔãÒ?Û[órö9$?³Hƒë´"ð?þìÔ	{?¤7[Ä°{?ߗ¿¦ëß?¹~qL­ßu?ֈÉï??´ù¯¦°µ=?À(Ù=—À?¸e@ïBõF?ʲçÀ»i?Å{tñÕ¬?åq\öÈk6?Ȟ/"Áµ?·™`ݽ?Áõg~Fé?àTHȁõŸ?Î~Ûüq´?Ùsˆ©(?Ë«µ'6>?Ñw&~*8Ÿ?±5
wŠø'?ÌÔ;R]è?·=®
²?àfòL6?¶è'è?¢òëvYnH?"gÇZ48s?ä&ƒìwü«?Ùä.àŠ'?ÕTš¸
ß"?ÂS¦ê©ÆQMIXED4FGL J1814.2-3000¿áÌ
õÒT¡ÀΡáf·ÅÀ:ØC1­÷õÀ<mCÖïe~@0ÒĚ?ü}s]Å­õ?Ô»´4çh?瘒üÕ©@;YÎy@TÀœ<â	?ïýî½ãOñ¿èø¥˜«]¿Ó/ÕÜ¿çpi§Šô¿çg'…€Þ¿ïÉƽ¿ÐUNASNone?çÀÇQ'?ÅÅÀ|e÷?¬@Š+4³?ÁÏi.¶?̘Ý"º¹?Ár£>;­‰?à]ìLø_?Ås'«¶,?Ÿ§Ã"Úý?žÌ^gê?ÝäÇ÷Jó?ēG¹Ìv?ëBà8J°d?¥_PáXšØ?£<î½ O?"˜z3œŽ?¼J†Ýz?¢»Îé*Ó?è‹Uï©NK?Ÿ,Ež¾É3?«±ÿ7 Xº?ŒŠEH"(?Ææ(s;¶å?›Z¼ÞÇ?ã7³þtº'?ÄÀÃê{Š?¦éÇ|2?¯è7XÔ?ÖÎZß}17?ÄB™F|Tÿ?Îm¥+ëb±?Ã]w:°;X?§½†ÔÓ©?«ê¹Ïrƒ%?æèŬ(*?Æ)ËDP?ç™Ó˜Ï?®¡Ï°óK"?°Ã²a›H?Ÿ€—°/?Ëk¿4Èà?ªîh.æ½ý?àéåÓvy?°'j/cù?´Ý8¿X? 44Œö?Ù¾Ÿ¸l™?°@òiû'~MIXED4FGL J1814.4+2429?ÓTW=²Í@22ç³ØàÀ:vÉ5h—™À<‰a=2@'ìðٜi@Yã¡$¨?Ø1#ùÚL?Ó´B|Ò8œ?ÿàç6Ÿ?óDCƒãNï?åÉl|«¿ã¤­><%Ë¿é²¾=èÃοåq؊p0ë¿é+·sŸ4
¿ïÿÈ!ÂGŽUNASNone?êº dè7?Åqº«?¼â?¸s¿3×ÔÛ?Ä}¨—ŽQ'?±»@jJÃë?¯Â»™!8Z?ê,.<?Åùhê­¼?¹~³9ý°?¿N1]½lÕ?µÜ3/ò?¶"‹$ž¶]?éÕ¼st}?ªßûÅç3?²Çy`³ð?¡}›^±4m?¾Š£_<?¤o<ÀÔ?æ0K9BÔ?¢	ï;8p?À´'üëšæ?œ.ÜâC¬}?Ɗ«×YÌ?š²•ÝÛ?ç\~,oŽr?Å\¡S–?Ã7öœ)ù?Â
ïd)?¾¬!d1`~?´Kœªá?áI0?ÎóœØ›ëŒ?Ñ롏Ãh0?̏Í
ˀÙ?ÄpŽEÜ
á?¿xȶ	3R?åT£šÆ·¬?³ƒ
%!?ÁÍ´"ºs?­h7œ
7?Èß®àÂfÜ?¬Í[‰…Ó©?ÙÓôª‰$?°;yƒÈ£¨?Ì/M[¹ ?µ2uŽ-œõ?Ø!s­¡¹N?±y9½;	kAGN4FGL J1814.6-3621¿¬U?ÎQP7À!ëÒRGËqÀ:±šW.ºþÀ<,3øUÔ@dn¾Ï‰?ýAŽXø?ÒKÝcß$?Þ¼Øc@§"©GŒ‡?þ<sÿP³?îö+jçÕg?ï†G½Xæv¿×(èÁõÙ6¿Ë1··¿êJë€ìúj¿ïõXÝç¯UNASNone?èAÙàlÍð?½èðCõ?šÑĞÏR?'ôlxúÔ?˞_ë¼ÀÕ?»<åN"ø¨?ãB–Ðé×?Ç'€"'(?£—R×
O?¤¢Ÿ5B?×
àçÍÉ?Æ¥h×àô?êͨaTûý?¨Œ•F›`?£žØÌ!?"ó{]$‡?¿Ñ툄†?¤³'u/m[?èg,#kâI?¢s+(wÃ?²Ó_µc?"KÅwö?ÄùÏf|ƒ+?¡\…¡~»?àØ9‡,¦ô?‡"5£ó1?³d¾Z>?ª³D;h¿?Ùv][óS?Á…<·¸µá?Ú>rtš9Z?ËFlF¶Xþ?²;(CK?µù–?§?à™aŏ89?ËDú}VP?åõª
|Œ»?±Û×¹N¡?°½ì5ýü?œ…;´N5I?ÏàøÓ»ÔW?°Fô7‹6É?ãè+ofã?±Ë5e2L?»îâÚÂ?¨¦Æ¨Æ]G?Òöw#*°
?³]ã\.Ÿ¾MIXED4FGL J1814.6-2537?ïdˆ=HØÀ°LÎå«ÁÀ:qó·ó ôÀ;±rGE8ï@Ï0֌"#@x~…A?ÛÉ{"P?æãèb)•Ñ@ãÈ\$Ä@ÿ[g¯¼œ?ì'1ÆK©L¿Ê™ú<œ"t¿Õyëñ@¿çýB`wº¿ïÿþˆ0»Š?ïÿ£ÿywUNASNone?ٍöm…¦?Ð7iÐ(L?˔àR̼Ã?Æf†`›?ا™iù?Ì4¢Ô«¾_?á¶S°p ?Æ¥î€j?¡qõª¹?¢IgÆñh#?Úc*~¦©?ħ"œhÆ?ÞÔ{܉?²á‹­''þ?È!<?N@?¬6˜¨¹åB?ÕՍcˆï?° v`v¼?ä`äÎ:$?®MµSÆb?¯Y6Ä`L?'bÁ©¿/?ÓSŠ?<4?­¸+;SNm?Ôåâl
.?ÒNùv½»Q?Í­±SŸR?É8p:`à&?ÜCDê&
<?Ð?í&š¯ª?Î"Ù"4w?Ãw^¨¤Eç?±Ò·yQÆ3?´‰¶ÛWè?æ<òȯ³?ÄÍtE)ÞS?Ñg^BnÖ?²?"q?ѸÁ–Ó?´ÎÎ(ÉK.?Ý|ƒ7Û?µ€boܒÛ?Õm»Èv.Ž?²‹öžM ?³œên¬?¤†Ï<"¯?âÕ¡^M×é?´ÿÐØþ'ôMIXED4FGL J1814.7-3420?ïVöҍ^«À uæ6*^À:xv3cÀ;Ñ[§Æƒ@®Qäy;Ö@ëE®_ú<?ÑgC:è3[?ÞcK©Í@.ã,?öVwî¤
?ïã&@©?Ô1½|Í°ø¿áÜ4-n¿ç<¢³Ï¿í}Sþ.ïÑržƒ
fUNASNone?É98æ{t•?¼h-%}$?Þÿ¹yþ§?ÅlÐbÙi?ÔcªºG?Á»ô5OÖ?»B3/œ¶?»ð¶\¯»?ÝnR¡k(?ÉBÄ#Zù?ÛÀãàd¯,?Æç¹Ï¼b¿?Ñ~~³í¶Z?°!/~t"t?×IJc·Væ?²[SÅäT?Ö¼ÎçH?°ÅëBiî?µ	uŽB;?'Øiì‹b?çDž?©ßʙUvá?É,^­µZj?¨l1ão)?´ÿ›óÒOb?°ŒJ ?ášá¥u9?Æ*H¾_̙?׊U¸ˆ?Ě ¨‡7?¥Às©ï?®"ôŽ5L
?áù9Ë0s?ÌUfŽÕEl?Ùm4[|RŒ?ËbªÍ§ê?Ä|H\Ýs?©qŒwV«?ݶè7??¶L(EÆ?Ø
óšR7l?´YäÄW‹Â?•Zã¡0®ø?}/´»ðo?èLuÐwãM?µqJÕÄ?Ì"ÌJhPn?´Æ
u´bPSR4FGL J1815.1+5917?î¸!Qg@;Ÿû¹IbÀ:áZˆâ'1À<D|	f@×lu:(@¿\¢˜F?Ðb\ªŒ0?æ­z¹Â@ê±ý=­à@áð˜XüÆ?ík9i®ƒ¿ÒîÍþ¾a¿è̀†£пêòI^ãL¿ð?ïÿ±%§YvUNASNone3FGL J1815.1+5919?å!úYU?ËÊ;›nÜ?Ṉ̃R·¡±?ʪgi™ï?¯ÈUÃѲ'?¯æmbÓ
´?èŒúôAI»?ĝžŸEˆ©?ĶÅæöæô?Á±y¨@.!?²*œŒ˜HD?©‰ÒÐûc?ãn0üù|?³@Šԙë?͆/:©}?°f››u"Š?ÄÁ
p"?«ƒƒÅ
?ê~™ Ðoš?£ƒzë¥øD?¾¥$§ª(ˆ? ¨°ã¸ Ã?ªÌ§QR?ŠðÜÛêuJ?åÑ?çæH?ÌÄ`' ×?ЇIG>$u?Ê­'9€ª4?µ\PâìTð?¶Êà—ª?ÝJbªCž?Î01"Y=«?Úx•R¨?ÎÄö²¬î"?Àz³Mu?´ièôB)?Ý›Yüå]?µAŽø–l?Ó;‡ëqR©?´ÃúŸ¦ ?ιu#ô?²ÓPž5Ý?áã¡ÙÓ?µô€Ÿ‰t?Ô-(ˆ›€¶?¶†²Gw?ÃB iŠÆ?¤h®ƒTAGN4FGL J1815.3-1336¿àyòAìÆ?ùæŠÁXÀ:µc#»ÇÀ;­iiP%²@h½}¤p@/%¿­*?Ն¼RV9?ï‹'!­@ØÜ@Þ¡@Ѻü•½A¿äúœl²±¿îd%ÿn	É?ÆÔ¨Ž¿äJæ
²û¿ïÿ¾[ðÁŸ?àRâ¥üÿUNASNone?µͶ˜<?°W»=XP#?µœn^
*?±J8¶Á"?꫘}B~ˆ?»]&™YF?É€ÜfüA?Å<ý4QHû?ÈWx¤xè?Áç»è›VÕ?ã©ÁŸÈê?Çÿ0ë7úv?Ր¿¢º!?²@ï¡=F?ÉH"¦ª=?¬žŒíj¥[?ÞS%m'R?µ »qN¯?×0¨CÖnŒ?¯Jن]ß?Ç#ñÃk?©ÆÛ§H=b?Ý=ÍCGÛê?±žCÅ.?£t®,Â?¢Ç6
Ùé?´±#®Bäz?³ ->/?ì2™ï)Õ?·Ôm·rÛZ?¶Yëý«?»ê§"­Fu?ÎÚÀŽ·$?È÷ÆhøM?å~Lí՗2?Ê#·cÈÁ?ȧuü}â?¬CÁó?Í*v\cê?³,ª‹ûš?⒲DéǍ?·+VrŒì5?¼Ãv¼
є?¤ª›åó;?Ï´‹šIå?·<pÜ|'M?äznAë̆?¸
ˆÃS>OTHER4FGL J1815.8-1416¿ì¾YÂi?ó2±-4À8¯Ö»cýÀ:<òô~Â~@ûèɂ•q@#¼ª ?Â-«3õÐÒ?͍eä@ûdg?ìiZ"›õ¿Ôû¿¾òCª?ëÄQh¨`¿æ9œf¿æ"‰!Q^l¿ïeDþ6ҿ撝'uÞ©UNASNone?«
þ,˜e?²ßÇN#H?¶Næ&–ëà?¹dÙhNŽ}?ë…CX;Í®?¿Ð Va?¥«þú''?°^‹4ÀÀ¿?ӑå*f°ä?ÄrÏ'n¹?äÜMŠf9µ?ÅC±´Ý0·?ÀÛ¦ž(¹?§*&ò?Î¥À®ÜKñ?²»†Þ"å?ä6ê¡bÕ?´'.ìG?"7V-‰%-?y!hT?ÈÒôGÿ·Ê?¨&Tx^RÊ?é1ˆ<"Èä?ª™ØQçß? °D¡ï?°ÕRNÏ?Âö 3¸Ox?Áä,öê>?ê7s²‡Ú³?äÍ\ó)?•YAIRW±?ŸºÞ~D?Öp°˜Iô|?ÊPƒ>þo?äÝ©ÇlÄ?Ê4àòɋ¥?¶Åɚ? mXyçî?л±®°¤p?¶`ÑW  ?äɄEŸqu?¶Î됓RÜ?wµï2\«?d'ØÁü?Îê>_Y?µ{˜
zÈ?èIYŸÐâ¨?µÏö‡Ð&OTHER4FGL J1816.1-3908¿äûèÎWˆÊÀ$ù³ÃçÀ:Q¤nß±¬À;ðbMÒñª@P‰áÿº@
vÙ{0ù?ÌÂ*7‰?ÐGýûCÝ?ýVÝA‰?ò¨"pÃ6¡?ïýê|
<š¿åÁ`>¯¿åáù£Åm¿é=b.$¿çû¾Aě{¿ïñÁ—ådUNASNone?æíÆ8ÖX?ȔñŐԊ?³‹äÓ%lÑ?ÆQ¥_ܚ±?ʅÒ
Äw?Á"yã¬ôQ?ä'|†8hÒ?ÉGR¾­"?£µw'—?¥€xv¹cÇ?ÕOD¬éi?È

?ê+íä@ÿ?¨§"îh?¤¬-0iô?•ÛÝ4CÁ…?ÂM]bÔ?¦f§€—R?åÉÕ€?o?£F ­?´¬P$?'Jq{2õL?΂¦üø±?¡E€œe?âU1Êê?Æök	kí?­ov>ýj?º=ßP'ó?רÔU)?ÄvõŠ†+S?גćr¿T?ÌÉw9¿¶±?³ú%ÁŠÃK?¶¬'OH?á·Yì?ÌþTñÁER?äpî™K?²Gœðô^?³b1G¡? 'ÿ¼ü.Á?ÒGkс´Ã?±Ž ÒÍ?ÙÙ5³7œÇ?«ˆ¦ºæÝ?Áš"œÀѨ?¢àJFó¦?ÝYþgúe?­_èj—`MIXED4FGL J1816.3-2903¿ïæó£•	×À"ͅYÀ:"Ü·%››À<opŸM8@*ÓÄ[d@DEª.<?Òäç`Kð?ïÿûÎBÓ@Èd©ÍÄ?þr¥;¹>¦?ï'v1µ"²¿ãýô·ø¿Ò™#"™Þ¿ïÿâ£Î¦Â?ï؊p0ꄿïÿüoQÇsUNASNone?Ýø0:&ä¾?͘4…ˆ?ԆAj%>?Ï.•RÓT?Ë·h.	?Â|Lr°‡Ù?áٝÍ}CD?ˊ­,**?¢f¨—Ó"?«
¦˜¢Ò?ÙÿïQºh?ÉFãÜ#?Þ­™ÎAù?´°LìöA?ÓìՂö6u?³ûê£u±?ÊË![ÅM§?¬c˜6Þ?ê—";?±¾`}ÞM?£šDÓ-^ê?£&tñµ¶?Álí5š?«"'j^I?Ú	ã:™ÑD?Ë&µÁ:?Ҋ_VŸ|?ʛ<k·?Ók½nÇ@?ÆPR¦ž˜e?Ñon€nÙ?Ë¡ÉBB‰?·/õ®é?À1˜fÇ<ô?ä—å*wÞð?Ë$
óªÿj?Ö¸Ç'­;?´¿_'JH?Ú"ò¤5?¸1ß҉?ÎH©\–j?°´w.âJö?ÜÅZ'ŠÆ1?ÄeCN'æû?š,D4@?Ã
ï®ñg?ÙÙXW@>ñ?Ÿ$ÂpíMIXED4FGL J1816.4-0057¿ïC‹j¬Ç@_¾vÈ´9À:.Hè§À;_WƐr©@ïxŒÙ—¶@ˆ¹º¡Q?Ìzº0gý?Àÿìý)·?ö©Ä¿¸T@WKÐ
!?ÜA œ,ÆÝ¿æރ¾ôÚ¿æ¢:Að:e¿ãøèI*}¿ïüŽ[wõÛ?›^L€PJUNASNone?æl~x«ãH?»æ˜Ý©`X?`ìp€l‰?vèÉ|/?қûªl
ü?»Ç
DϾ?æ¸q<?ÁŒN#ñÄ?›æ0öíݔ?št¸†GB?ÐкwàŒG?¿@ükî2?è6^¦©wˆ?«ò›aAz? î-7Ï,×?'In^'ý?Êêúy7h?ªêåÖLí?æ‰ÅEf]ú?¥À'cX?"u
CEæ?q1y©¤ö?ѵ$£èí?¥C<ûêä¾?ÚxÙ,xü8?¿íå$¡8ä?—³^\nÐI?Ž|:ñÀ¥?âøv"Â?À1R亐p?Û&¸¢.¤¿?Ç0{†;Ìg?§®×ÊOñ?ªù›Qž÷?àñ¶2s8?Ɨ×å&,\?àú ̝
?³¶Šlà;?°"4òËÆ?š""äœE?Ú1*øÚ¥?³PŽa!ñ?Ùëe©¨–?°yÝßï?¡³3}î³Ë?‡ŒQõö ?áïóhX?°‡8@ÐÙMIXED4FGL J1816.4-2727¿°ŸÁ
Y!Àªä>šÀ:EžG~CÓÀ;ÕbþÒÙV@týۅ¢@58[' N?Í$ɍþ?à†ü©3j'@µÇ`c?ü÷Ǫfp?ïœQքܿá÷ ¦éŽ¿ãƒ>
É¿ÜÔ»%_¿ï
•µŠé¿ïÿÍ'ý UNASNone3FGL J1816.2-2726?¹˨QƱ?ªÝv-¬?๎‰#L?ÄD7v}¤Š?ØKñ+¾[?—=ÒQ?Ï$ë²@.™?Ã,Æýªæ?ƲHo¸þ?½ëßC"KÉ?âŠ2÷´Ô?Á[§¾~?ÓneyèŠ?°"öm¥·ï?Öñç²è[?²FB…?Õ {žd&?±hÈTè?ÌÛôÁø!S? g8Ä"Ìa?Öù)'ìj2?ªŒ…Û‡áÇ?ژÜ…$?¨€ŽeöäT?ªzn>Χ*?œÔI•Å?à.¼'&š?Ň´÷?ÜS:*¯gG?Ä|ñhôœ[?µD…9<?´ã¨ŸÈ'?Ð!©ºñO…?Æ®sè§k?åFš{–Ï:?Æ(
¾ŒB?Ł`·>´à?ª1œÆyëa?Þ	e>Ò?¸½:-qX?×4Fˆûf¾?µà"ç:IC?°' û'?ªu7G'?ÜÔÍX5[?´š!ŸH?ß)Î>«¦%?³‰ãÌ¡6zMIXED4FGL J1816.4-6405¿ë'A‰jÕêÀ4ŒfçÀ:V#ßÙÀ<FÒä>@$þØ;–@›¸€®?ÀÇÐy)·‰?Ö°Þ$
%'@÷jøœ^p@eÍ=`Ó?ïÞâ¾ÑŒz¿ÜTµ"0ѯ¿à€ÎۚƿåÖ½•!e¿ïüK_ÏÉV¿ï'nÂ6ïUNASNone3FGL J1816.0-6407?áVHÅ`?³©°?Õß»&)?Á Ã%{‡?À™ì¿u:.?°Hxl¢ö?ê^Ùkãö,?¼*ŸÔy?»Á
.šOÖ?¶‹Ç^
èµ?±H'r³òM?©ë¸É€T3?àmG>5?¸á"f \?ÔUºr¾I¸?µdBƒ^ùó?şn UF??¬÷83·¸?èbiW܉?œfñÕ¢Ù?»_ÅwîÏ?"@8Mh?ÀÆwäú&]?"è"?ÓxAUñà>?À±=áH@?ßó3¹¤?Äë|t^s?ɈíàÌ<?¸^'¶¸n?äì¸iW?ÆNáÉwòo?Îù‹Q'S­?Å*>ÂÞau?À²dûœö?µ*ší³uƒ?ÑëK@Mր?¶	•‰w_?߸–½yÑ0?º €­~?̸<p° ?±oâS+R?ޝ
áÊ#¿?©Á—Ežž?Îg/Ë/û?©àò­2Ýá?ÒTÁ‡c%?¥
Êë=~¥MIXED4FGL J1816.5-1208c?èœ"e@Š	¾Å£
À9>'lVjpÀ:¡¨žð@þÓ xñX@!Äüó0?ÌòÇÞ%²?ËáÌ8RVå?ú€yK!@»t_οïòbüO?îþýÁ·Dû¿çIðäÚ	Ì¿áÇr_Ãßé¿ì|vÕIs¿×8\OUNASNone ?Îão8û|Á?¼‡-A'Ù?¸ÔÇq\þM?°ˆmÜ®?å,‹C•?ÀÙÊ_ææ?Ô°¯.´Ò?ɉÈ
›9'?·÷ØK'"?·¼®[B|ï?â©Ÿ³5?Èæ¡vÕé?Ñë!–Ó––?±Gñ
XÐ?¿ºÞ£8ÿ¦?§µ!nìp!?ã`/Á?²R—(Zz?ÔxyÔ,g'?§òVŠm…?°y"á©Ê?j·ü'¥®?㴐™¦ëÎ?¨L¾—dg?Á);3müÄ?°Ôð©«"?¹"3Ÿ¥Þ?°Ù¹›÷Õ«?èƒNÌõDC?¹ëzÞ~·&?ÅjìªZ(?ÀH"íÔÉ	?Æ?r€>îl?Æ2¢Ù¹?åh5YºB?ÈÑ}‹›ÿû?ýíz±ò?¦f݆q?ÁÿÀ[
£Ù?©¾ÑÁ?搔‹ƒm?°n»"	Iº?Àl²¦Ú?¡'ÆüF?¶ˆæ'@›?¿FˆlÎõ?鶃èµê?¦©)®'°OTHER4FGL J1816.7+1749?Ë>ùåߘV@/M߆ã´À:GI¡À< SúSÕ@@ƒÊû;u@XTŠ›ÏÕ?ðHÔÛd?Ðv	ý.êN@OÈ‹ñ:@¬ß¡GŽ¿â-ŸàÛwŠ¿ÝAÛ¢R¥¿¿ãßKà(IJ¿ÕÎN­=%¿î«A—z©¿ïáØݧ:—UNASNone?êV…æÖ±?´ü"{&Ͼ?²_Mu
O?¥}Š°¢¾"?ºì'…çò(?°ÔÐЈ0J?ëÍÖw›m?·3…rÙ?±:Æõ÷?¯ä›Åt½?°WH}|•m?¦­ªG¼­?éìþ{Ïõ?«BzÕcY?·z?ف2'?£½?€½bs?¹ÌIPHE?¡‹Éñþ?êp¶tNd?–©:È,e?¬Ø;§â6à?ŠÕ­ƒ÷À?¾.Š	·A?'x´íiÈ?ã®2"˜½?Á
ùâHxÙ?Æ¿™ÑnX?· Rš|y•?ʇž¢öm8?º¯¤Éd?æh-ÙWË?Æ­fÄÉâÑ?Å"i;?Âüý_DfÀ?Á<ߕš?´FÊJٛ|?å­¦ÁË<?´Cnóž_á?ēîƒo¥n?¬ûYp<[¯?ÇZá‰-¢?¬z 52?ä`íçµÃ?¨ç^Q!¹A?¾´`bsñ?¢Õ³X‰$?Ð"&
€·u?¥'…³dš)AGN4FGL J1816.8-2800¿ßéˆåcOÀq´xB1À:fVߋÀ<
çbzH›@ë\ђ.@ý'$ZR\?Ô¹A?:}?ï¬Zœ-Ȑ@ &5?þOL'S$¿Ç"(GÔ?î¼ZYê
¿çoÚ]ÙúÞ¿ïӃüº{?êÿ}úâ~¿ïÿ:Þ"_¦UNASNone?Ú½MÇøÁa?ÇSÉÆ.o?·NÜ	åY?´­"òÐö?ßnû22N©?ÇgîPÖ\?â‰TbÐ?ʨ'µµë?¡¤´Zß l?¥D£gá3?عQO¨ß³?ÈiÙ9ºg?ãªÆ2‡oS?±×ð\úå?ÂûiÍùów?©Ù¿šýJX?ÎY}gèO=?­K]ы[:?ꔿë?°éÓ7Dñ¿?¥›q­cÈI?¤_Ü´vi¿?¿¡)õ‹¢?¨Õ²ZS?ÑÙJ0Xk?ÃÐÓï£2í?Àír»€Á?¼! 6+`+?âØ;~8óš?Æ[B(QO?ÒOOÀÔé?ËvV=ÏCu?·£K³?"'?ÀÏ™!?äîáŽiª?Ë­Wüì$V?ÜJŽÎ([X?²làq"	É?Ìf^‰æk?±¹ùäö?ՂB$'±s?±f6¾‹Ÿ?àU/‹'?ÄL<…¦?ù/¦5ß?Ã+oáJ™h?Õy#
#Íî?ÀÁ"—H¨ÞMIXED4FGL J1817.2-3035¿×‹xÉëF
Àœ…×EÀ9oßq?RÀ;¸ò–Šñ@Øä|û@؛7(‹?¶¢bk/å?¯Åäü"Ì?ö-$[)'@²¹c
–l¿ÞBkØ?ïÿɯæ¿æ-'?2D÷¿â§Òw0¹¿ä³!96¿á'‡N={UNASNone3FGL J1817.3-3033?íÙÍ
?¢^õ¥P_~?ovٌå?g/»UhS²?°;¦ÃOØ?¡Õ¢ÿõ‡?ì¢òuJ?´Ùm&ñqÍ?dö(r†K†?oàq÷i…Œ?ºHŸá?´ok¨Ý"Ë?íe'#®†?›eß̼ƒ??ˆGœþ8=?€ûõDÀB^?±Îì~«È?˜1J¥À™c?íÏÞUœzÜ?ƒ%$:f• ?'HF.§L$?lÝd7u¬¼?ª]÷ŽÅ5?~öç8ZÜ?ê™ÙxÆ?²Ý'Z¦?ŽwUÄø‡?ŒÇ©×'>*?ô?ýµ½?²Æ³?ç¹í!+?'nL'Ëfh?x˾9¡f?ŠŸŸíñ‹?Ñe],UôS?ÅKfûâ?馅1Ïþ?¬Ûkû?•±?n0ğÕé?Ž‰ž©í²r?ÈŸÒmˋ?ªu' ?¶?ëæÑ'Fã?š`øpóà?¤÷"?ˆ'¤Ü.CÔ?½MG퐢á?•>K'CîkAGN4FGL J1817.5-1034?åþúÅ¿£€@³	ý¯Ã¨À:ÇíiûFÀ;Ù€9vC@©Š(b@ñ]¥Í"ƒ?ÒáO¦0€Ñ?ç»ÿTßUf@‡0[žŽ?ö7–§¡Å?çèQBgك¿²ªËÁµ¿Ö§e47?1¿ìm² {¶¿ïÿþó…õ?︣µ|N/UNASNone?ÀÖˑ'I?¼üÛó±=$?¸Lô"ÇÃ?¶s'‡Nþ?èÇn¥¥?Ã)žK§jµ?ÌT5è«`Ó?Êû4IÛÂ?Ñr=¸Oð·?Çc¯sÿ?à1Ó©­/p?ʹêß~͈?Ò3%æ][j?°*nÿÂ6?Äþ¢Ò?©#$š¯'V?á¦å$1—?²\$ñ¦—?ÄÙiˆ"ÉS? »Ô°Z¡?۔".Öà«?®/ãâœ?ÙþÇ溬?¬–lÑUÞ?³D·`œ%z?´ˆúœ¿?Â2…ݾÑP?¾ ž0,B©?é
ǜaJ?Ã_@Á?´†ÕéùOÚ?¿â$Å(¶?Ö²;?àÚe?Í^(Gzp'?â¢ÐhÒ?ÍH"Õ(?ÄKVž$÷9?¦³6ðd?Æ{0A©?¯>^ܤŽ?åkˌt±Ç?³0Ž»×?¥E[6®ÿ?‰K×y6Z?Þµä¸ü¶I?¶5Êð²7Ô?Þ¡oß¿vV?µ¨æÝêãUMIXED4FGL J1817.6-3251¿ÎÈd¤*¨[Àžm=ðüWÀ:Ò7yêÀ<€Èþ3:@hÆøL'e@ÛÈ:–ÔÃ?Ö¬]᲍?ïô×x!yÍ@'ƒ'à@_VlHS¿ïöë¹÷Ýó?ïÿÄ;-Óx¿Áí@	Û¿íO9ßÞè¿ïÖ´!…5ß¿ëœm‰pVªUNASNone?ǖ¢'ÖJ¿?¼²¿3ËÎ9?Ñnp¶vt&?Ä®n®Å‹÷?ác˜£?Ç_ÜÃ~´*?ÁWÞÕ;;?ÁÌë;Þå?Ü»`À×m‡?È÷{þdZ¯?ژ¯Ô™tÜ?Ç2ÉÆ?Ùµ†òDwö?²ßi%–9?Ö1ƒ~,ß:?²Jéë
!?Ðõ¡‰Ž?¯nô÷°?Òy©x£™'?©‰<m-OÐ?ã	Q…â5G?­|	1tDµ?½ÎÍêl…? 1–ÄàÁ¸?µO.
†??¬ÁÊrüã?Ò:»«¶Ê?Ç'¡‹E?ä8¼·«ÓX?ÈKsĦkB?´.ìê/?¼òÐ'ÜN?ߞê¼Kö#?Ïl²ªPÔ?ÛZɈ'^ò?ÍY)©1£?Μ]{'µô?°p›[ï¶?݃çy)T?¸[×I¹™?Ó-éÉC²?´÷›?˜‰?»®¸©nÅ?¡{*BÉ©?çHBä×´?²5èºiú?ŘìäM?®ma|M¬§MIXED4FGL J1817.7-2517?íHTyóÀª0À'+çÀ:–kÅJøÀ;¾}ík¨Æ@‰+Îdý[@º"¦6?Ö<€"Þ?àþ!†ù"@
X¥ÛÇ;"@‹4ԝü€?ïç¥*ÇSç¿ãe•®×ï¿á˜aÁ;¿åzJIˆà¿ïÿÿ" 5•?ïúµK¦ÇUNASNone?Öñ-[5¹?Ä~5?¼7ª{¿&?¹'i'Ä}?át*ãó?Ær"àªÙ?áÓ/{Sï}?Åã«Ë—»?3_[Íç?žjZô/ý?چkŸD(?Ćú)@/	?àQ7©ÿ1=?´qÛ]Gÿ?®[y»¢?¬¢íá\‹M?Öbï}?¶?±~å•Ö?ãUe…ý=?­¦q26!ê?¯J÷€A¾B?E³¢áM?ÕkÖ D]?«ÙÀÐ: ª?Ò™^úûù?Á¯ƒ`"?ÇÀøåüÀþ?ÃK7ÞS?áuQÄ?Ç=R"9éŽ?Íùõyê'?Âù(Ívn?­oU
xž?±X½ëLX?æè'M^œ\?Ã¥[€Àk?Õá¤	"?´Øhpލµ?É© š6D?¶94ÿÉÌ?ÝI‹—ÖÔk?µÄ»7º[¥?Ñt_'% ½?®ÇÚÛ¿j?¶[È°L?¢µÐYdÄR?äzW3h?±㙙£èMIXED4FGL J1817.9-3334?×bZ]n›À 'ҝÇ%ÄÀ:Ø"r8À<(ÐV©Z@RȲ5ò«@–¦ Z?¸m]ôþ?á¸W=Ôw@ 7 þ}I?þÀd*
ñ?ïþÎ!`¢Ø?ÀÄ,[Ø¿ÝÿFÃ*¿äu/dÊ¿ð?ïíßlÁÕUNASNone?¢äJϲ~?£ß'×Â;}?럢'Õ?Á̆Ý:"b?¹ÉÁá~Ž?¾Q¾µC)‡?»«&c/éì?º]8ˆeG`?àkÎ)e¡g?ƀ½½îÁ?Ø=šh·?ÄôéáÛ|¾?Áƒ
Ê<l?©l	ëwÂ?äbÚŽ%?´yœ(^&?ÌñŒ×‹¹ÿ?±#e€?Ð#["D=?©5‡ÁíÛ?âŠá>ž(?®ð;¼Ä–ó?ōÄä þé?¢°3|Ñè?"Õ]ÊH~˜?–°iûØdA?ìє»A?ÀA>Še…Q?»ê'ŒÈ?½]b~Ü!?¡'S
'ú?¦p±[쵬?än×N0¼?ÉJÙ±Ñc?ÔòY¤ë?È\ktÜå?±ò‰‡V4»? /…êÂ?æNXÜ¡<a?¶y?¶=-!?ÍÍWÈOß?µ2?G‡‹Í?¯ª&mr·<?"i†à
O?ç©
Ù-ù?±'³p[?Éq?‡Œ?­ÄìDæCPSR4FGL J1817.9-1135?ï÷g!4Å@+àXšËÉÀ9H¬A<
À:ºŒã¨±e@]ÆYÁ@ßú¦ú«?Õ4<Ëbj?à÷–oB­ú@
ŒWâ?$Ù@¦o¾(ð¿Ö#IüMmò¿Þz"@Ÿ¿äkŒ–|¿ê¹ÂÅâοèkœ0LÏ¿ïÿú¡œGtUNASNone?áÜ,±Ë?ȧ²¿ý?ºFÂ,ñáÀ?µùmÜÕÃ?×\—tj#ú?ÈÆ>N€|Î?ÎáJÅd?Æ 5Ìâé'?½jœ€ÿ™Ô?¸‹Ž®¢øå?äšeÝ]m?ƹø×;¤?Óýþ/gÄ?±[ªø?Ğ×âæ¥Í?ªm!^¨	§?àÙJï'tŒ?³-3€:A?Ánpò—Ò?šh`PG¢?º#¿ç?šõÑÓǽÄ?èaÒ"Õ ?£VÐ9qn`?כûBDâÍ?ÅvqÊ%[7?À…;ڇܔ?¹Zœs\¦Ç?à³h;—u?ÈZ1†­%4?¶.ÁZ§4?·¤ŒéÕ=¬?Æ|…çÞ?Âõѵ·(î?ç›p~å†?Å;Ab½÷?ÈoüôüI?©ïécY·D?Çk9ÙYfè?°0xÆ·Ë8?ä	2ƒ,g4?³Îÿb8hÙ?¡€ëwݲ?"ñyÝðV?½YÝ8w7;?§#ü؄ñ)?ëC|J9›=?§®
Dó)MIXED4FGL J1818.0-1339c¿Ñ8ӎ»wÃ?ðWš5 Ë½À9?Ùx¬ºÀ:ZaՈ@­>'
@¸©õ1?ΟH/Cºj?ØZí!*È@‡#uP@î›×6ˆ'¿ïæ†|†c\?ïú^À՝¬¿à³%³A¿æ
ŽÏ;<¿í<ÜÊpÑú¿ïì¼Á¼ÎRUNASNone ?Š pR??z9Á¤?zRêó#Y¿?z™Œ¤*ї?ïŒFð6?…a>÷F#ú?À1µf¡2?¾Í‰ayS?¹HËبo˜?´Õ–V
|?èÊy+B¬?ÂK¤Aó?Àa(ypÚ3?¥mh¹G¢?Àá'(I0‡?§Þh|Qpq?ç¯l'}R?¯ë¢¢Ô?¹YB)†'?¢êuÉS¨?§Nø¾Eµ?~ŒNU?ë_ÞkŸz?¨{Íì1–ü?~•áBz?z#r}x_8?†ïž²'òó?‰cöY!Õ?ïh8Ysõ×?'O" '?²AkŒïPÖ?°[wc€=?‰}ö-¢?À¶e™Ú(¢?éð.É
?Ã(0ÜÒå?³T"5¶¡?—yèÓb`?¿™–êg½T?©&«SÁ£?é¢<œN»á?­òB¾p²}?¥|·,¢?•&³T?¨'8¢s?˜¿×^Éè?í%Ø1.÷?¥&é'GêçOTHER4FGL J1818.1-2000?ٟ`ôÈ¥‡À	 bvÞÀ9æk¤"ÈŸÀ;Æ¡Ú°»@)²~AúK?ÿ)¢üê³?ËæáK	Î?âÕm…>˜Â@)4AP,h@ŸJ(Åò?äT´W‹P¿è4%CâX¿Ês4j•Ë¿ÓìöÖBL¿í#¼Sƒ¿ïÿ·`)
UNASNone?Ç.î"N¯n?»´<³µ¥?Óæ!0–¹?ÂÈÁéü?àA3ÂWÜh?Äi›.ð‡?ËìOú?Á`/ç4"A?Á9_XfZ?¹]>ý‡Mé?äÁá+Bh?¢¤'‰?×£ÑxO"?²¢´ã/?Ó5ìKV?±z_<õ€?ÕÉ&B<™?°˜£}ÖÑ?Ü`?ÔÏ?¢Ûûnç?Ç%§LI?£;beQ¿?Ø
a‡%ñ?¤tºwk¹?µ¹4N8w?«Ðâdœ^[?ÔµÁԇg?Äe½@Š+4?ãBþ•Û~?Å3d¼Gð?³ŒÈ'óû??°J~Öl*B?Y§O®?À€"\Ð?èî'1]?ÁKšÃç?Ðö;—A?°ˆ0
bÎ?ÖsÜ՝D¹?·Š¥™ƒÔs?Ùn,îËz<?´îî4czr?Ɏ[ÇjÑõ?¢»A»àa?ÐÅ¢2ç«B?³û;³gÿv?á9—ô±uâ?²ÀåîSRMIXED4FGL J1818.3-1233?å+UÎ釙?÷Û¼Ú'.À9'0¤ãy·À:¶]këáe@ G9Oó@ݙÙZyÉ?ÊüÑâ¶C?´Æjˆ	#j?îXþý–ï?û´¦xz:¿ïç܈+³?ëÍ$ Ҕ?µÖR²÷¿æ­
$F0f¿âù!°:¿î³©æ÷UNASNone?ƒ¥‰'ä™?À®û3E/?'Fh5ɤ?€î$µêѦ?ê<üñ¾Û?À_"?Ò?Ë~²òtëÔ?džTsÛÖ?žÞðnp)?¡ £üƒz?è,DKßQŠ?Ǩ äwÊx?ÓÁ‰³Ù?²a†"ôj®?µë]@?£¤dÁÔ(ê?ãԁØ:qÉ?³?]-ś?ÐæóHPj•?ª·Ø²©Íÿ?™ÕAFŽˆ-?'_P|€d?æ½ÜQz$?«JsüÝþÒ?»~ñÞ<?°³ÁxÚ5?ˆ-ÂRlÖº?†Á%ÕSc?ì/jÓÕÌó?²Y]<¼·?Ã"l´[?¿½;èÁþp?¥9ž/¡?°eø\'‰?éé§JԆø?Áøÿîë¹*?Ç;!bÀ~?©ç;*Pö
?¶È1S"d—?§éÔ©ìÌ?çX1|Ï´^?°Ç	Œ*L-?¿ûHåeä¥?¥ úožþ›?›é†‡g>³?ß‹Q"¹?ë!J¯j€?§JÀ
cÐ;OTHER4FGL J1818.5-2036¿±â+ÂqAEÀl²
.À9ŠºÅ­À:Š@aïß!@
uΎBù@¢ÍbJ?ÑEäü"Ì?Ð0üw?ùúYÍÑ°?û輻@-?ÑE0¡2•)¿ç.yÖ¿èÿat¿ì<ø¾îì¿Û¦¾%6™¿ãi¸ËŽlUNASNone3FGL J1819.5-2045c?ßls3¦?Æ0Ì]ˆ"¯?•%:"Sô?"aøõHÊ?ßA*ãê†Ø?Æ.…[k'ý?ãé.xŸŠ0?ÄrroM?'˜à؏§?"B¢¹iGá?×!€ê\f?Ã_9wuû?ÙNÙC 
C?²Ò­eU#±?·9?åéÁ_?¢ù5Žì½9?àqka;Èó?²™I"ËÅ?×ݺ֎?¶?nÒ\?—+Æ­Nk?}½¥ì$?ãWÄÁªH­?¶Éöï-?×¥—ÿ™?Åy¥LD?"þ±q#D?"åçÔNÇ?ãɸ¶yŠ?Åò2ï¸×o?Òö°9Ýá?Å뙰Y"?¡N&IWò?©)fDÇI?åâÅbþ°?ÄþíW$E?Ò´ËÔHµ?±9ÆeΒª?¹A!QÚa?¤9	D•l?ã}uë$âÊ?²ËˆŒe…i?ÃŘê¶Üd?¯~dÈwå?Ÿ¦¦èú?~ÚHîº?ê|–³?±£€ÜHÅMIXED4FGL J1818.5+2533¿ìœ‹¹dÄ@2$Édb€(À:>"i®ðCÀ<ôËÛk@ƒ¸x¬äû@é/n'"š?ÈHLŠr4P?ҋÃbjÙ=@ޓ@ºs@Š]sùvú?äþÍûÌ¿à)F Mgè¿é±'IC?ñ¿ç-'àAõ¿ì`½¯ùWo¿ïþV²"<cUNASNone3FGL J1817.7+2530?ìf÷A%Ë?±>lÏ-?¢ÜÚj|ó?ŸJûq'ùÉ?²&[&K¢?§Ù€óÝP?íæ¡H?¨‹ã̹C½?œ§Îb9‹0?œPÆÅ`l³?£Bß æ?ž%ҍÜ"?íÁ¼
?¢Â|òÜæQ?›n§ïð)?'\ML¨¾ê?°¬dH:<£?oúÀ¤@)?쮖žðú?‡àÁÁîÝ?¡9Pàk†?w
U¥KV?±ý®`ú?'{·š¼?è^$ŒbŠ ?ºaÎÒ
¤I?´0,2Na?¨·ògi…P?Äo_9݂Ž?´íÀK—Õ‹?ê9 ×ó¿?¾'måÙ¶?´@ߺ?uo?µÜ-™Q†l?·ÅS?ÜӚ?°Úª ž‡Ê?èØq–^?°ý¯‹Ñãk?²à";mÒ?¡9sû5§?Ð)÷Råß?ª ¬Êƒ.d?æûÑWԅÜ? `ûáU?·.|æCN?"'±UÊx9?Èy|Ù¨?›Õ؋³,AGN4FGL J1818.6+1316¿í@ü(sÖ@*fZUÖÀ:h«=0À<€à,@ÐøÇÒg?þ7Tð]?ƎNâ¼"[?átÝ!®¦q@mÝS,Î@¡ÀM|€?ØîBþ­Dœ¿Üô[艿ЏÊB®Ñ9¿á›þÝÁ¿ïó6>¿ïva0FšUNASNone3FGL J1818.5+1320?׊âî2‰P?ÊÁÛ!yLr?ₐ"3?Í5¨GmŽ?«ß[¶-P?¥'µº?Ôk¡òŒ,§?Æ77=´?à¤ùÇVÁ-?ƺ¶]'V?ĔÔýŒ¡þ?ºšT%Wc¥?ÖÑ3i8þ¤?´Šy@ ¾ƒ?á™	><Þ?µ-2Záœ?·òèk«ù?¢Q·Õ©F?åª+Kˆ??¤Qàõ2ü?È8æÑZÑ? ðÂ,WCU?Áԁw
þ?—x¼þnG–?ɉC[ۄ1?½fJ3B¼?ç
Œ!@?Ã-¤Þœ-?´™<Ó>-?­¿váê?ÆÇÙyi´‹?Áօ¨¤?ä;Pné}ï?È(`=Ï»·?ÈJäÊðS»?À¢c0•¸Ó?Î~ðöͧ?²ª-<Æ|H?ågÞ9lïS?´˜[ Í…þ?·ÂR<öœ?¢Õ¢>›Ö'?Ù,Ií<?­ïp&P?Õ°0­OŒŽ?°¹Ç–¿æ?Ñ#?Ã6æ?§Ú'ŠÁˆMIXED4FGL J1818.6-3206?çïO¦†gÀŒ†‹ŸÜÀ:#R©@À;Ûo¼P}Ç@—%'Ænd@˜{0›©?ËJ3•XÂ9?âîA'šÈ@å	9d¥œ?ÿiÅHŸ6?ïÌ¡-â'Z¿¬ñu?
e¿á±Îyu6ä¿è™¨èÁõÙ¿ïú×lbÿª?èøª O€ÇUNASNone?ͨ[ö˜D§?»¢ƒœ×?×>2Úa¥?ÄmØ=ÌÇÍ?Ú
"ÐƛI?Â{4B–—J?ÓéRëp?ÆjrÃy+?Í4þºZ¯N?Ã
'­«¹?Ý|-¸tü?Æ1Êν4?×7žz²P?²¯ ä^?Ô-SŒçPÿ?±
ì[@?!?ԛ
÷SLó?°•j3E>Þ?×mݦíGÊ?¨˜к?׃ÿn_¯?¨±5ŠÍå?Ñ"ê³	$?¤,®Ëå.3?µ¤-žk1õ?¨fØv׫?ÚÞ|Ö?Ç	ü$ •¯?àBCk?ÆØ|zÇ>?¼¼Š	ƒ·Z?»‹%ÚÒkj?Øe¶°">'?ËZ÷êù?à5"f¾iÌ?˽-¦	<?ÇèöS;?ª/Å< ó?Ý<CwÎî?¶¡«4?ÖÏA€Aȑ?´cá"V¥?»Ô¶ug?™áŒzáÃ`?àµóÑbL•?²Ée§3<?מê×#è½?°ÊPÕ1TŸMIXED4FGL J1818.8-2255¿ì
P#êüõÀ0U¸™9"À9×	—XvºÀ;>|2€…Ì@š¸ý·ü0@÷GMœk?аiϘ?Ò «†+(@wºÄŒŒk@¶¤¬È"?ïɯa!¾¿ê~Åý0¿à"7É
û¿ãÁ9ñ"U³¿ï÷Q۔欿ﴟ¿x{gUNASNone?Ø|\z‡ä?ÁÖ±%$?Z"—6æ?'`ùþ}Û¸?ãx׿f2?•
"¬Æ?áYSçÄÛù?Âù~µ×V­?•tà"º=§?"Q¼ª"¥]?Ûö
''T?Âh;ydA?âg§<š™?±<õF?±ðxÄ$<?2k¯rì(?Ö´"œÑÀ?°i}Á"©á?ßbaÆn?«Êµ¸Œ'?¤ƒfmO;?]_NÐ?Þ
{Ü¢áJ?¬"\Ÿ×åô?ÁFk섚?²*Sd?›sµ"Ò·?'¹°ŒÁ?êàиØ$?³õ¢À'ÿ?Ïmº"L8ú?Á6N®¥´?NŒÒw5à?¡6O5[ý8?ç:ô'sb?Ác)²£MD?Ó€àÌDM?°¥|%U?¸Ø1îRá? 4¨:~þ?ãW¹R«­?²vBÝ?ÎÀ¹»'Ö?ª¿qÖP?ªÇºQ:©K?'ÛÉé
bN?棁,˜íÖ?®"ӒÚOÒMIXED4FGL J1818.8-0828¿îiýÌ#Ò@
\‰ô
(xÀ9e(ÃnÀ;=ˆ ËR@¹·_­@Sœº¶?ÇCŒ^?Çãv‡pÍ@7}_§/"@"؊ñ
?ïàƒ˜¦T"¿êF]ýŒ2S¿ãq
‰U~¸¿Ý:(e#ñ!¿î©"ÿ+Ý¿ïæítãìUNASNone?·Y@ˆzE=?³aÿÆSžÔ?"nÁð?Š7V®b~z?ì|¤xŹˆ?´ã6ŠÝgo?à‡ýu×s?ÿÑÖeÁ•?±Š5û†ëä?­MjÌ9šz?ڍxG©%Â?Ág/jŒ÷Ü?ÝÞ´ÄuîÍ?³]±1^ôa?¶¹ƒelï¬?¢¯˜)D?Ürêc
¼G?²p€	'?Ôa܁©@‰?©Ì	/%H?­.¨'. °?‹dŸWlÐ?ãü'<ý-à?¬èw}?­)úׁ¾?¢qÔÚg‰	?˜{º#ã?"_ž·jÙË?íiˆ$¯ÀU?¨/¡–-Í?σ=jLX?¢NK3ýU?»Aè
s?º}¼29§Û?ä×Ûhhkœ?ē!V"1¿?Ò4꩒Ç?°MØAáQ?»vû¢«Å?£)Î<…ä¨?ã'"«6á$?²2jÁïíò?ÀþØDœ‰…?¢LÒéâÖP?³tõÇÙ"?›=÷q?é^[O±îû?ªã€
MIXED4FGL J1819.0-1203?îCÐÒjñf?ùé5¹qÀ9h™YùÕÀ:"Š.‹@ÖÿU¶ú@)ú}	@?ÒÐÏ:æ/õ?ŁÛw_‡û?öýŒ£ ?ûe¦MC?ïÐN+Ý¿éx¦¿òÉ·¿è ˜'[Ýv¿éþ_
¿âˊw½¦¿¿ïûï< UNASNone?ÖÆîcup?ÃŒî÷€;?•']h˜d?'sS`"	?ãðà›òËu?뤉×Ð?ÑÆV"mà{?ȶ?,:Æz?¢Àß®¦Æÿ?¢í€³…R?åðÆóÞ£S?ȑ·JãÒ?Õj	£
?³8Tۑ›$?²"}R³á?Ÿb;Ú,Îî?âúkÚ!Q½?³paÂsÊ«?ųí¶Y÷K?¢Xzq^ˆ?š©ùŒi?~ïh°|	ë?é¿BJ¨E?£Ý¾}ýÒk?ËCy&‡~?»®ÀÈ1²€?"K —ƒ¢‰?Ž§zéçK?蠒ÞÄ,?¼â±Pá?½IËK]?º;ø'?¥ÄÖÝö*?­·Ä4ÊMq?êú…åò?¾Ò6]^Þ?ʗçѵB?­fUå?²lMõÚs?žBÿ÷r?ç|kœ—a?°ãBï×ï?«ô†2á3?'þ8`¶Òy?˜öÌG
R?ˆMVuµ?íy:´ÿ?—0méºÍOTHER4FGL J1819.3-0935¿ÔLò¨ç"@>°YÏ/À9n*†¼GDÀ:Ç'*ç4W@áꛔÆv@‰1‡aˆ±?жšÙ4º?Òiëáºð@±îúôþD?÷L³è$l?ïÿ••_x¿±úfch¿êñ´âg¿é¿ü¿ç׏³•¿ïÿ!é^ÓËUNASNone?ŵºC¨ú?¿Fî±Ãå?e욧Éy?•b^a7½?êù¼Þ±ë?Àvcç?ØäúUœÇ?Ç$:^˜A?»tµßuq?³nH¡?à*4>vn?Å`†	'E°?֞Ù;'t¯?±ü@ŽØ£Ú?ÀÁ¾†ù'?ª¥5U¸ža?à€#À"G_?²ïÿՖR›?Ài§T~mª?š]i™tü?¸ñó"Pïø?"˜ƒ>ºN?èÇWºHˆ&?¢Ý›Þå {?¿f:\`‰?·6ÃanMô?Ž4Z]k+w?s&üȨ?ëšgJùÑ?¸]‡âMl¹?Áñܞ"B?¾hH4¾½?ÇËñ°†ðõ?Ã	T›x@?同lVâ²?Ÿᇳ­?Î@ŸÔ…¢?¬öLŸ?O?ÀPYƒBÙÞ?ª!\±†Ë6?ä[Á©¥wÁ?²C¡«Nz?¥&'Û)4?‰ýya¥œ?¹¤ôšàÛ;?žÍä­qÆJ?ëxþô3»f?¡óFS¢~OTHER4FGL J1819.4-1102?éÿ)M×#h?ÿ_ì»"À9¬m&SQÀ:žÄüô²Å@HÛìû@~@RiÄ¿¸?àôC3[w?ඥxÊìù@ûç¢;(Ë@£;Xñ‰¿ïðÞú̺X?ï7ÐQ¿Ø'k>gnÏ¿ê'ÂIÇI¿í}tՔòk¿é"[å$xUNASNone?Å¿-Gê?½Þ¿W]"à?ӎŠ%¢×?ǘÜSí+×?àÈö)3;?ÊÄَQ<?ÅY9>:‰?ÄD$§Õ¦?Åj?Â}9º{x?åhpô¬1C?È™ýÜS?Êjó«€CT?­Yßqúu%?Ȕ¶{os?¬&¨÷Š¯?ã@'AN?²œU*#Ëÿ?½ÂAŒÇ?˜>'s T?»¯¸ƒ®dœ?¡Ø6Û£?èÑÀ¾òt?¥±ï€õÁŠ?ÂE™ã҉?´Ù(Nùn^?ØøðXåkÌ?È»&fñü‡?ÝäBµ1O®?ÉVúžÓQ?³£#'+ÐÚ?´¿ÈåÌ?ÑåüýØ?ÊûF}ù}?äü¨œŽ8	?ÊÛz\	»?¾ÎlE^À?¢T;C¾?ÊG@4°?±ƒ»º??å"NgRZÒ?³0ø:KÆÌ?£(O®­Á´?Š÷ž"8Ê?¶	Ã
Hwo?­Ô™:D¥?ìB£57?­ø¿ä™ãOTHER4FGL J1819.9-1300?ß9Š/™J¿?íØ⟜èÙÀ8Ä,5èðÀ:BÁE°
@ÎÍ&8ú@×6žË2?Óí¶Üöe¢?Ѽ)çZ?ÿÄô@¯¹?ùŒ˜êS¿ê÷–¤ò"0?ÝîÅû¢MG¿ëõÄÝëB¿ê¯:J~©S¿àvÎ}üÛ¿ê¬çŸaÑUNASNone?È[]S˜-‰?Á%E–¯{Ð?‰Dÿc¶?Œ&|ý'Ί?é"Júz/?Á þªaà<?¹â†e'ßt?½¤µmX?³<+q+£?³žŸª	;Y?ê\)ϺÆn?Às‹†*?Å\#ïjÓÖ?««YS'6?¾ŸÓ€¬I?¨ap
?æÔü"Áê?±wŸe¡ÊŠ?±[Fi?'F0Yò·.?©i%~"°?xv¨5»9?ì=ÿÔÙX?š›1³Ò?µ_~iu6#?´sµÊËÂk?º%*[ô?'Å­ÞDûO?ìÝ'þ®?¶aégØÄa?­Xä^ï¬?° i"m?Á€é-š[Ð?Âg²ÛxÐæ?éÊ7n=?ÃlŒMß9"?Á4®A‹)ƒ?¦\@•îՐ?À"Œµ895?«~dùÔÄ?瑱BO'R?±§f¯,$?"G•&(™ã?~öíb'–%?¬-y•*9´?š&Ð;{²ý?í¢ë½RÜF?›Ÿ·³
OTHER4FGL J1819.9-2926¿ïÔ#FÖqÀñˉ֮À:ª3DÐêÀ;Óà{Ö:@˜p¤ý[@¦k|OÜ·?ÅÊE
K3?Õ[Á<ëÙ@g/3Ê1è@AyúíÇn?ìvµ~|‡»¿Ð—¿ú¬Y¿å7ÌÎû¿áFJÂpþE¿î^%"ôÆç¿ïÿÿ^ðP`UNASNone?äu +Õ­?ÁdAsðm?´Ä"~{?¦r쥴ˆ?Ñä·Õ	?¿£eút"–?ãȒ«hÎö?óö£F&ç?¢]ñö—ù?œ¿=í÷??Ö#jøt?Âh"Âç_?æû:,6?±W¥´Á#‡?¹çnñq¿,?£]¼×]à¶?Ç_ÙPá?«ü9m,?é¢%P¿?˜ÓzX9;±?¬ÓûL3¯?‡=Xÿ_A?Äv¦£JûÚ?"ìÐÎ93}?Þ%rs¡?í/¡`ëÜ?ÁkÂà~Ÿ1?³?†ùÒì?Ù%MJ?šÿ=jø$?ØH#Æ¿Ó¦?Èl4lÕR?±Ue"%ãÊ?±–t4h?á±AjrSs?ÈRÝûüþ?ã's+µB?µ"h'8ø?Àª[ÄÝü0?¨—§d'?ЇëÆ&d?²<v˜ï—Ö?à/Ñóìæ?§q7ÔòO?ÁZâ9E›ì?¡bÄO¸•?Öòêûƒeó?¦.Û3´ÔMIXED4FGL J1819.9-1530¿ïȼjæ#¿ÐWÁ•aüÀ9gLÖÀ;#ƒ×u.@FÞá¢G@í>" 
Q?̾­º¸Î?ïÿîbHÊt@Ôb^™éK?õ'{è-Ñ?å³ý">5Æ?ÝdZÝò%?Ѭ{ÃŽ¿èx²>@ÿîR¡)°Ó¿é©ÃGèÌÞUNASNone3FGL J1820.3-1529c?‹Šˆó1¥?'œ$Ö|•?äu´£òª?Ð0u–ãe?Ö8F­þ?ϦôOa€è?†ãm•]3ˆ?"€Í5v†$?á9u­k‰?ÊJŒHÖ¼?ÜÕúf¼2?ɺ8¢«2–?¸•n^ÿÖ?¢X#~E'k?Ù®ÁÙÿD?µO|ÜGß«?àñG;¹ü?´a]yº?jÄÀP÷ñ?SӋ™*ý½?êµî^u†?«gOú§(?ÄÀ#uiÓG?«l÷8Öí?~{Íoñ>?~ZŒ	®j?ã0'\o?Ë?T$Œ@?Ù]ðjO˜Þ?ˈH…Í?yîúËÜb?Šxç…PZ?ßóîe_˜?Î¥jâeÕ?ߤY&ÈýÆ?ÎdGNM?¬OõþT?–©™ð@?A?ÙËÀÏ#ÐP?»Vbâ?áU ?)zg?ºÏ•/Z>?C/kEö?8¿DHká?ëàÎüŸDÌ?°N-u‰?Ài"¡À¸?¯þ¨¹ˆ|…MIXED4FGL J1820.3-2646?êå®ðîÀÀƒëaãIçÀ:-îÉp!À;uñÀ¢@Óaš#Ø!@¢¢dCvw?ÔLÄô;Q?㥾/ûñ@©Ô•*™?þ"¡Û1"x?ïý
<(¥;¿Öy7¤\U¿éâL@Jrë¿êÞ́®Á¿ïá¤_Æ95¿éäL —©UNASNone?ÛàMäuœ ?Ʀ"êò
	?ÀÝ·Bn[ö?ÈDÅí4¡G?Û°ÖzS5æ?Çu¼dõ£?ؑ»=G"?ÇXcG¼Æß?Àwè'=?»^Z؂|`?ß2Pšã?ÄH<¯³·R?ÞFŠÎ%?³>A¿âw?¶Õ¥-^x? YÕG:iB?܁*H9;?³O¡enXs?дt
¿? vj»?Õ½†w—ªñ?¦ÆJuƵï?َo^:Q?¥2‡Ô¯¡?ÒʲÉÉì?Á†*Y£h?Å»0vž?Á{ºŒ'?áÖaýc?ÆR½ÚÊ?Ã*I»Æü?ÁH4rß?Íwè þ0?Ç 
†Ñ?ù?ãÛûk??ȍM}X½©?Ñ×&0Û?±½í}¨ó?½¹`€À§?¥õeï´]‰?ã½h\Ï}›?´à'Žã}Ö?²aÕ,I/?ñå¹lmž?Ü5õãÏü?²ùʬ'7?ßUTÈP³™?±î~ê"ÿnMIXED4FGL J1820.7-3217?ç}saÀ wB™ØƒºÀ:"Ô+|À<WÔUWJ@$‹Å¦Ê?þÖË8x'?Ñð\žçaN?çmjW@KU}
Ú?ÿ§‡ Q»?î[õÊd?î±ã<zÛ¿ÆQ$ŠÎÑ¿àGóÿÁ–¹¿ìUŠÁ9›­¿â]ŸˆUNASNone3FGL J1820.4-3217?ÊÁ³ì"Ÿß?»Û÷o<?ݶã;¤ý?Ä¿­=>­?ÔèBÎJ•?ÂCÍ#"´?Èâ{!€Ð—?Â+¤¸Jy?Վ¥Ë½>v?Ä×ì{ðÈ?Þ¢ox€?Ƴ°sÈ?Ùý·×®cf?³K6°ÒV‹?ÖÀ.Sz{q?²í½ÄWn?΄3©®BQ?®6 U8€J?Þ_°%ˆ?§µ\{})?×<·kf«?¬°ž*ëã?Å®Ç0ß#š?ŸH°½G€?¿¬À8¥õ?±ÁØ~«µ?Þ
›õiy?ŨQû,Ý?Ú
3ýêh?Ā!ìl'é?¹–EÑB™?¹.†Ш?ÚÄ#Ÿ)?Ì	bÈT˒?ÞÖK¢Q	n?Ë»TaMš4?ÏdSðÀÃ?²&'"wHŒ?Ý}]x×Y?¹Þ"NxLÝ?ÒÐxE?³†üé2#¸?ÐX˜Ç<Y?ªàøåÅÇ>?Þpô²¢‡²?¸	Ìíºö9?Ñ6s<–;õ?°âÒyö@XMIXED4FGL J1821.5-2531?ê-aÉ.ïÀ&,ýxÀ:úmïǤÀ;c\Äüô³@àû­àÎ@4@^"àÍ?Ìj(è¬|J?ÉÙ¢Ò1f@8ݗl@íÚ£úñx?îÿü¿¿Ó½°d·9¾¿ê$'ýuE¿ßL‰°îIõ¿ìòSš¿ïÿ7ûþéUNASNone?ÝC¥‹?ÁåZ§U?¢*˄É	?–Å®ô•UÍ?àPÐ¥Òë}?Áü_]¨Ž?áø3³5Ìì?ÁòðztÒ?—'½›ý-/?•3Ÿ¥Þ\¨?ږlÀ"ýu?Á&fïÖŨ?ä|0¥q"?±h#ÏC"?ªáµ†f?˜ŠqÎóo?Ó«iK"I?°r2hÜ-*?ã†-êQ?¤f ã•?°ùmԊ?Ž	át1|»?ÔµˆHʅ[?£á[Óz
ê?Íiç‰UmŠ?º×ÂȒ?°¡p¸mÒé?¤~ÞN̹#?æ'Xs®ñ?½Tžè¸æ'?ÑkÍýéC?ŠEÑùåè?¥	
³À¿×?¦ù«¥{HL?åùˆV"'?›ãÅP›h?ÕõQl$¹?±¦ía3‡?¶ùCň?¡_º ‹'?â&/¾Î²?²‹Ì;•Gô?ӊې´ï?¨)sK?ÀBöZö×É?£¿"—0›š?âbüûyï–?¬rk%"™hMIXED4FGL J1821.6+6636¿å4°k¹#@;ª% Jù#À;(o`àëhÀ<Öö¾7ޔ@ è¬Û•½l?ühžŸ'×Þ?ÃÈÃRЇl?¯©¢?g¹?íýú1@	ĺËÃbk¿ìÂmÎ9´W¿ïÿúâô?ïÿíUÙPi¿åØQÀ'ô¿»OÐ^
¿¿à^¨A}"ëUNASNone3FGL J1821.9+6636?â‰Þ:³Z5?ÕÌț?†þå¸Pö?•ðìcVl?Ùð"vM?ÔQæEÞu[?ïÖ@Í`ח?xÉï?ÿ?D¬ðð|?S¦õÁƒ?r[ã̇É^?u®(bmà
?ëtr¦É¢?¶2tZ¨" ?Kq"ƒéš?]t_6h=?ÂÄCÍpr?¶6Û¡`iK?ïÔmßÚ?Ypë—Á'Ö?#d|zéÏ?µ&=öÜ?u-ïèés?Y4Íåð?èäÿQ7?Íz'˜?ƒÇàYg"€?'u^5qOC?Îkíüi¿Ú?ÌnD²²¿?ïˆ0{¦r#?'±ä
£i?S¬ˆÏ	?dç´‰¬9?‹~PÔ3ˆ?\'%çMà?ê.øcÜüÎ?»9'~ú\?P2ß•ü}?[z|¯??Ç#¹3¤?»@Q~Í»_?ï~¼l
í?{\C	{?5k¸€|¡˜?7Ù͗œT?¥‡,'VÆ?{$;ÐÁAGN4FGL J1822.0-3146?Ì6¨™ÍØÀ ySyú—áÀ:•¨þ'j÷À;ã)þK@ႁOù@4Ÿå
5s?ÊoEFl?§¿^5{ž?⦓}æO@>—…BI§¿Ú
ý‹["?ïþô1•¤B¿è@C=¿Ý'œdÐK¿ëëÌ!+HÙ¿y¹!/‹ÅUNASNone?é&ЌAd?¹'"ÓÍk/?Œ9ÿ8Ê?ˆö	fn ?ɤTË*ؓ?¸ÅáH2]p?é'Rݿۚ?¾·Úóè*Ý?qúíQ³?zqYpËûZ?É2²!ê?¾)±ü&4?ê-"s¨Õ]?©L…¤ ."?–܉1ô?ŠÛ[¦ü ?Än]è"î?§Ïv=õ?íb¼'FÉ?‰	Gwá?†&^L?g3æhRšo?²&úmSqj?‡\:°®r¿?㉤¯èv?Áô±ÅVÙ"?¢@²Ò#?ž¥C©ŸŒ?Ö¤´É倒?Á¥šÙµ"u?âœmlr¢'?ÈÂ(å7t?zÁ[¥NJê?‰Ö܃¿Q?Ú\¸N‡ð?È­ÚêØâ–?ãÊýÀU?´qú¢=Å?¤[sÜ*>Á?"0"Ž¶—?Õޗt=¾?³"FÀÅÏ?éNx³ðÝÎ?¡¾ªŽ4z?šgÕëô9?" ¶nf?Çy"sÐå¿? ÕœÈ*Ú'AGN4FGL J1822.6-2502?ÙR•
mÒÀ½Û˜A«À:q7öçRŠÀ;…yB=K@ÞM¨ªY@´ì O*à?ÕÚ/¡XTÖ?à"Ìô9ù@Xæj,Å@°
©¶È¿â!֝l¿æð+¬V4À¿Üɀ2Wk¿æ®°:Ê¿ïÿϞcWé?äæ»@2uUNASNone?Ý)ìU±Àà?ŦçfgNT?°:F†w(?¥<%Ñ_~?Þǒج¡V?Åödî
±'?á4nBdÙ?ÆΟ"aNØ?¢wjœ`[P?¢íÌ4iÂ?ÛH6'âУ?Ä÷†‡z?ÝÔÑNÍԛ?³3<ë´<µ?º'9ucü¡?¡Ófè¬?ۆ RÆK~?³O¢ž‰?à fEI?°(Ëڗ7U?´xà;9á?–Rm.XbU?Ú¡½²?¯Å©Îi1?Ç4bü,>€?¹Óú~
òÍ?½dɇŒÀ‡?²x¨¶>¬=?æ†NXO?Àà`è³ç?Ë搉5Úi?Ãß '&ûº?´2~;åÌ?¸«£.ß4°?æ€MøË?ÅK‰(»¾?ÐB£B_e?°i¥üå‡?ÀB ñI%Z?¦±öûù}?ãÎõ†÷?³ÖcŒ\é<?ÄZÊ($-Ô?¥ð£Y €?À°\FÛdH?¬¾ßÄä/œ?æ½6dɋØ?²…'·¾kãMIXED4FGL J1822.8-1118?æùóZ}ã?ñ&Y0þÀ8çíåÀ:TK8ãv\@±Õ>ì¥@ÃJ‡ãŽ°?Æ~Jž3Ý'?ÂƇÕvê?ý¹|X@2ö?ÿì0àr›ÿ?åxÿnw­¿äƒÛÂ3¿è%Ò݈ó¿å'úhçJ'¿íTvyÙಿïóܦ^£úUNASNone?£ÍTj½‹?«.^›Gˆ?ˆdóøõDœ?‰±k'VP°?îa–é™"Å?¬±à¡æ¦/?Ɵ¿
œi?Á=4™E?°<-ïn»´?¥˜¼¶':?èPŠ~k`?Â/‡ÆÕ´?Æ~ÁØc?&?«öï#þ{µ?»*•R&?¤ˆÙ'Ûž?æû÷<ëv?°™ˆq#ë?Â)VÍ? ºâÔúá?®J4Á"«™?‹,ÜÐý"Q?é"RtùS?¤CÞã6ÿ?ŸÝB1r9?¢HcØ'Ú÷?'æ‰Í£ÖA?'×5ò°U+?îiᡁU¼?¦;AÒYò?³áyVÀòr?±7mÖLqU?³MÔ#hÚ?³ß)ÈZµ?ëRìz×?»P"–JYÀ?ÄM÷Ž,?§þ›M/&?·Ö;à
ÃÎ?£Z³itCç?çñö†è¬?®óç…ð b?© t}v‹?'g‡Én°?²…')ýnD?–Ì;,{Þô?ìFrÍt_? ©¦;þOTHER4FGL J1822.9-4718?¢†:5=ËÿÀ.,ê(þ&À:cÞº5"À<6%ðT'R@þ 8¯žê@!%‰Õ?Ãÿۂr5¨?Ñ'ýž%ð@	N½ÅÈ̍@¡ØàVls?ëJ%󯏥¿Ý(¸ÛÔ&³¿ÞÊZâN¿+¿äÁtæX¿ïÿòɶ—׿ÉÅèª;}UNASNone3FGL J1823.2-4722?í~³šPK?¤KpN™+? ú#0—Ö?—œž¿oØZ?§¢Æþ|~?™eÚ½_ÎE?îp²\q?¦í×Úå?"-¸õÕY¹?'­|×?b.?ž¼e{®?¢%W-»?ê…d"}uÍ?©ÖFG\ìÝ?²"ûŸk?žý¢ù+ßß?¹@à]âÚ?¢óÇÔ¾©a?ëâÍq&Lµ?‹EBz/
b?£Ìݶò?{IŒQ	Åj?·"ÎK?…–Q‡ÿ_¾?è0(óÐX?ºIf2[iU?ºí¡T_9?°_c½¿"©?ÁÈö²"?±¸þ2dE?ë¯V˜Ç	?¸é´£?­
› –K?®†ŸÐló?³ÿým&ê"?±yR´'JC?æ1{R«&?²¸c?¿Æ‡õh‰?§5é§ì0?Çq°hà` ?«Äñt?æQ9S2×ï?¡½ö¼§"?µQMî"?"}ª`øN—?Ìs»õ <?Ýzûæï"AGN4FGL J1823.2+1209¿ïÆßëb@'eÿ'+¾ËÀ:Ó°QlÀ<ª¾
'*:@­B§šcC@œa½Š9ª?ҖÞ­?ïÿ¤%
ւ@D9ô"?ûfkâ|·¿ãÉ¢
cB¿âɹòÕu?Çñ½_œs¿éÒ¹
x)¿ïþdž;îÄ?¸xQJuoUNASNone?ΐ˖ä*?Çôûמ¯P?æ='Ïè¯?Ì7ù+$›ì?°ñÒY*s?»þÞ­Iú ?Ɣo'¢e?ɨ=$½hp?æµ·ÃŒm?̂–»ÌR?Á
±o+å?¹ý{°rg?Õi'ÄcÙ?²À¬Uy}F?ދx(ۖi?´i"to'?Èì%'›{?¬TöËz?Ňö®ós?¦p즤?ææ²læþ?°Ù€˜dè?¾™\®'á*?§rïÂÀæ?Ł†r?½Žx˜
u?ç"¡Y£Ø?ƆÊÈCXÎ?¼Ñ.ÂqeY?¼áLqÙÈ?³4ÄÓþ.?¿ö€Ý,Ê?éA&9`Úò?É£RA¸©w?Áa²lN]?À¨e+)Ø?Ê«ªŽð"s?¯‡ÂWw?âýñ|¦ç?·àрT'î?É\~s߇?±ŒPÎj)ì? ¦¹œ
?:4ªÌ?ê®âÄ(Â?±ÊìøNKa?Á÷οQu?°£'þ»I|PSR4FGL J1823.3-1340?ÓþˆImºÌ¿½kW½VÀ7d_4Bý¬À9Ðè±.á•@VIã£Ô@0k_Êjó?¬b¡œ»­?ÏWŠý@Áæ??öÍþîˆx?êÔ½‡	Ÿ?Ó¸GD7<'¿à¤¸F-
û¿ã!½êÜ­¿ê
Ä
áj¿í¼ã`7"VUNASNone3FGL J1823.2-1339?t–+¨âR?u:i¼;ïí?Ö†žÁ»?ÎõGÙøL?äÇœýžž?Îí4ZiqÍ?‰zWÜv==?'/'Ô¾s?äÛÇò¦ç?À}Ւ\þ"?Õ|[+[	?À`ÿHÅ?§¡°'¥ Æ?œ®3x‹(©?Þè¶o4¸'?·ÿ"V[×?Þ#~?©—?·®ºïRÿ?i«æÙÙqÁ?Pëþƒb§h?Ó/£¦ã¯?­å¯üþ?æN'E®Ï¦?®*È
Rå?kh¸Ÿœÿ‡?dB´×ùÖº?àدòª	²?ɑ×+S'?ÞΩ×æm?É{ Imÿ"?w†Ž[lG?ÐYÜÕð?å|rŽµ1r?Å Y@&û[?ÔªøÈdn{?Å¢ã¢Ú¿?ŸÃªJ}
?"l—]J:?á÷É·]h«?½"¾¸"c?Ú1ì]Û?¼mÆéDÜ?Mÿ*ÁïT?;&\ðÕ	?Ö* "'Â?·a9¨X©?äã/óÒv?·—ê'¼xMIXED4FGL J1823.8-3544?ïJGgPNÖÀ$³H+è¼À;!<ÝÖàLÀ<­‰;}…@³GC¸?ÿŒèæÞÆÊ?ÓÒ\Ä&5?å±	!ç±U@HŸž–Xœ@µy'=/?ëLѿкî?íVˆm!k‹¿Î-º"{*¿àò÷ÙÀÑ¿ïÿŒri©è?è»K€1ÈUNASNone?élÇd5½/?¼ñW"Nñ?½/›š'o?³òÇö2Ӑ?·j)Á#ß?¯ÊÙź?äk4]÷úD?ʤ¿»Iö!?²yÒI¦v©?±Á¹&àf?ҋ"±8zN?Ç©'¤V.?æËx¸½:!?²¸¾+õ&?Å$+•m?­y°Há?¿[äëSö?¥8ÓÁi´}?ì€föÀLr?—Œo³˜Ó‰?°@ÀzIq?'Ÿ/B©A?§x…NØ?ˆÇq¹þ?孂å֑¥?Á픜Éh®?'ÅWìÑ?¸!µA^ÒÆ?Ƹ/¹¶›?¹Æ"ãmçÔ?ܳ' ¦±?Îaïb'¶?ÙZ¦áù?ÁÞ·ˆ?Ù½°²oR?ÍÎÝ!xe?àx»*Ä?¸JÛèRø?Ò%Ö_-ô?·~º•†:?ÉÔ UWlÆ?¯dr/PÇ?籫ý°€¢?­]‰îC¤?Á
6)1ҋ?©c,¯~?À,à*í?¢½j¹o=tAGN4FGL J1824.2+1231¿î;&L	ì@'Fd+ùƒÀ9ùžã…uöÀ;°öüK?™@²è @¬6|"ÏU?Å]b[¿ÄQ?Ȓ›ãö´þ?ýF©î@tÂâ¾%À¿ïÿ²'ž«Q?ïÿú Âî'¿é3¼$Þܚ¿çn¦`ýEæ¿ïõpŸÐ?s?î"úÎg׀UNASNone?ì9XU}?»A•{…e? µÇ¦áðd?®w"°ƒ·?¶ÃQh.eå?µZ¸|@"Ü?íƒrï>oZ?´b‰ƒ?ØÝ£Êû?¤!h.úÐ?¨Üb>×?­A®¥¦o?èlÿ³1£Å?®å¸} ÄÐ?®s·!ˆÉ?Ÿ	8®ŠQ?Ưk8I?ªmԃuL?ì°^¦˜I|?˜±(ûx'?œ>اÃE?+IÛt°?³mTÆoªL?".¿â×ƾ?éXÂBŠg?ÁFø7Õ½?³ZV"®ŸÅ?µÆšçzã?ÀïË®®m€?º[v2â*'?é¯k¨o L?ÅN4ztÕ?³²²©NÝ"?¹ܚã?¾Ñð_?¾>‰z'˜?ãlpíu?´{çÊ,ž?ÂþCùeB?­¢q[ ?д¨·!rt?®V=X¸ïC?ç6{ßõH—?° ONôd(?³[Ԃò»?é"UŸ¿?Éxƒ"Ÿ‰É?¬"KHaAGN4FGL J1824.2-0621?â9­_ô@ÐD¡À›À9F¿'țæÀ;Òê šª;@ݕܠªZ?ú7#¸kì¸?¾‰/¿
l?ãaŸËŒÜ@!gÛ	¦qï@>Ašÿö¿îYÀGƒL?ïñs	â×Ñ?Ä+üŸã‹¿Ô×~×v¿èUæ¼b~¿ïÿÿ" 5•UNASNone3FGL J1824.3-0620?™yú!W?šØ"µDm?î±sâ>¾?§¨Æf¹ïç?ßÑuÔî?Ÿn&÷òˆ?«0A´?º­¾a›3?äôè#.G*?ËÒåq®ä?Ò°'˜¨ái?É
ޫ؜ ?Ðlºd6Ù?°W3_×?½?áí\ó²%?³¨šïÁ)½?Çrf¼nþ?­º¥tA'?º;þÀ².³?–Éûdb?ä½ö1céù?¬âž¢ñEÎ?Ïê'Ú@Â?¨J8ª¸È*? èÜσžK?¢xNֈՀ?íôΉTA?°ÙӇ.¼?Ÿ¬¬Î;M?¢bÔ¯›îÆ?'Ñe…7Y?¤èohä2)?ç\cYQç?Ì¢h¡?Ð5ü7Þm?˾oÐ%$…?ÑRÉ×á4?²F>'ʸï?á5ä9¿®?¶Ë;Qa?ȂÛi?+0?¯çl™n?¥ÁNá?ŒÌÐ$[")?åÈ\î 0?¹$úv®Q?Ñ·"YNÙ`?·HIÊî3 PSR4FGL J1824.2-5427?à1qo·|À2Œ`Ëò²À:[ùæ
‹tÀ<‡²ù¼ïà@¤lŸ:˜W?ü~CÖ[?ŋ)ÿ­Ê©?Û9»n€'@Äq´xB1@ð¾'u³¶?îy;àÖÄó¿Î¬xCˆ–¿ Ó¢ s4w¿á™i=[U;¿ïêúêíID¿ïÿö$´ë/UNASNone3FGL J1824.2-5427?㫟x€Å7?Äùøè<G?ÓïG2eû)?ÄþCIMHU?²åçrÏÝ!?©OEV"¾?áTÛm%À?É3o`ú°?֊ååU7s?ǵ^dAü'?».KAô9?²-|ZC˜[?Ò+J€±K?²ÃÐ ¬?â˜JµÁÿ{?µIeZ¿í€?ÁH@*è`ý?§€ñÅCc?æÖٖëa?¢P˜I½':?Å'DÅ?B? uA¢Aî?¾ú«F.&s?'Äb•Øa.?ܬg#rl?ƞ;ê¼ÌÏ?Ý%Öüí?Ézņ÷?¸¸\³?­èkbë?Öî'D+lÚ?ËÛ[õû?àwa¥%?;2ž±?š"'·?¸Øz¹†ST?ÃÝ4'h¾t?°ÙB'Pï?æ G.xõ?¶!©¸""I?ÁJ¹·œ9?ªÂ °Öuc?à§Á[e½…?¯"éƒ;?ÏÈ×ar®?°»oT½Ë?͘#0ö[Ö?¤Ëh'ÂhMMIXED4FGL J1824.7+2403¿ÌVñ9¤Í@0HÙºÀ:œÑ¦PaAÀ<\G4q÷"@Sûª°Ã?þh¤~Ïé¸?ÕH 'Áç?Ù¯}HÖ@‹ÔÝ<†™@a4-.6t¿ï§x_7H?åì¡~ji¿Ý¥a~õÿ¿ã'&"©x4¿ëȽhÖ®¿ïÿöÅĚÏUNASNone?íâXwZV?¡äŒÍ|vÓ?–ìämž@?Ž'п°
ž?¦dNsŒ‡?šÃKBbî?í¬#<£§î?¬Gwü½«? ¾Üàpa ?¡½Ø‰¶¦?¤~ïUU?œ+Õ9æ}8?ìGÅ͐R?¥l	eåM?¤—£~­™?•E~i†d?´áðôŠž?¡"ÞQYŽè?ë|ý·?Ý­~›¯?¨z™·í.Ò?…,*6|—??·á³:Þ?‰=è8hE?êA¯÷Q¾?·ŸüËàA2?¯
‹}	?£_¤¡Ò¦•?¾kùZ¥
?³FÉlÌÛ0?êŸ[eÒ?¾¿ÉÙþ8«?µÄyÌʞt?¶¢	JB?¹–‹Y¾Kû?°cïÜ6ñ0?èÉe…A&?±íâàÏ'	?°`b&¡æ€?›pܒæ¯?Ī:¦š)?®Û¸KV,Â?燪%Øם?¤$v‡à??°v´#sý?›ÕLß<ø?É¥ýU*ÔÀ?¡k'27®ÅAGN4FGL J1825.9-3153¿¨îñãþ.ÔÀ"ÄÞÁÁ×À:"×`¤…†À;¾k#d‰@'ZïÅZ@ù4ºð!?Ïh`fþ?Ò@âô,@QáŽû°æ?ü†WÕÔÞ>?ïœÈùµ½¿åX=˜çÿãó"Çz¿æ:´ÒD2¿ïû]èHS?~+VUNASNone?átìˆvS?Æk+XYš?Ÿ^zà‡D?"9诉?Û F¨A8k?Æp'"]^o?â	òfÜ¥T?ÇÅ"'Ö­?«ïô¿æý?®áÚñ•¾u?؈3";˜?ÅԐMôW?äÉ¥ðŒfø?±A؋ž?¯Ö~©³™?™i–u•–?ÒqäIý5\?¯	Ý_®À?â¸ððK4º?©µQALa¿?ºáè°á'_?—JUÑæ?ÓÕ£ó11ô?§N[3¡P?ӇÊ{ÜÚ?ÄK~xÖÖf?©?Ä=Áˆt?¡@ËÊ ?ä¨~_\?Ņâôg¬ž?ÑÓt/Á}}?Ǿ¿»8È?¾k(åHç?À37-t®?ãS¸ƒ˜%?ɉ–ÝËx?Û`¼^Ñ­Ã?²CT|Á?¹ÐpRDèµ? €¤è±?Þ+'Œ?²Ï¨^k`Å?Î?›¶D?§F‹‰ôP˜?Ç£¦ôÝ?¯Tä¸ð¯¨?âªÏ¯UB¨?±é:1'MIXED4FGL J1825.9-5614?éùÕ	°À2ì|ÇÑ»IÀ:tý£.mÒÀ<W¿Úv@"¹._cé@\á>iÈ?Çòfh?Àkj1L(?ðu'a¼³z?þ±Naaï´?ïþ'¸«­˜¿äé5¹pß¿å¨tþ¯ž¿éžƒ¾ôÚ¿à2Ô¿ëÉú?KÅPUNASNone?縷4&^? ó¤Å?PÙ¼ï
?c2<Qå±è?"¤db{o?|¬ÇÞK[e?ïsÀN/2?Š!Ñgåb2?pÚ\7Òiñ?vȉÙù4?Š¢¾Erd?"EÌJÃ^?îÀi˜†?uP´ÚZ?}¥Òbe^?y])°a^û? J5®7¶P?=¹a§D?î3ßö¿'?€ÌUݚãæ?")‡ê@åF?f"=SßÜ?§·ž¤[Ė?}0!7âŠ?îáïGºÃz?—œ&Ø*$Ì?gÕ^i¶]»?ieèøႃ? cµ™ðЏ?–¬óœ"­?î`^ÕMyÛ?¦GpN‰K?‡ €ÜMp?"h>YŒKC?¤ò¦éë?¢!€æìÉò?íU6æq
´?žEUcx"?¬ùB­–Õ?‡"ÅG½ñÍ?±+
|¨§?™Ñï%±"I?êÑøÁjæ?šÅ.rÚ0?›d{ëãÝ?…Õ6q¹Ó?ÁDs'ü­?˜5—".AGN4FGL J1826.2-2830¿qm¬wâüÀXpƒڑÀ:zyöf#KÀ;åµWeA£@á]'£]@\¢}méè?ѯä^¹É»?ávU⊤3@«4<Ëb?ó|¥³Û?ï";ÞþR¬¿Ð»ÙÊâ¿é¦î¡ˆÑJ¿âTÿ5Õ¥¿ïÿþ½à ¿?ïÿÞr¾"UNASNone?ٕ€e-?ȾÜ`àâÑ?×û)™"ó—?ÌQ¸L•¸l?ÌÞ¬½´?À°ôgy›?Û ;M¢¹î?ËQeQ­5?À-ôô¢î?À‰Æe³Ê?ܙ-·âô›?ÆÚ^ck=?àyÂ*KFê?²Qí;4çò?ȹø0J‡?­è°ñÚ5?Ò¯cQLè?¯£^TÏ.?×ÒBš<?¬Ÿÿ×ix?ÓnsÏõ:?¬:lb~Ð@?Ô¿íp¨¬?¨æŸì÷?ÔÄiõDò?Æٗ~"ä?Ø 1a)™4?ËÄÓñ¦˜R?Ód©'£?ÅUL£Îh?Å"µmò?ÃÛlq\'?Ï^˜JÓҔ?Ê<ÞÅ?1;?âæø¿ïğ?Êó»
²›?ÕZd³f|ê?±Ó£x"›?ÑûR]è5?¶Ú&ìAÌ?تHî±N?´)'Æܨ?»XÙ–sI?žŽ—b%Ç·?ÛêìÞ÷-?¸±Ä(
6?Ý>ÜÙ#6*?¶ë@>—<MIXED4FGL J1826.5-1202c?ëN9
_0Š¿­Í¶<ù–ÁÀ7þ)›Ú¼zÀ9îõì@ß·Ú@¹Æ_ËA²?È
Áúá³?Û«;³´M@ϱÀo?ûFîK¢•Â?焓xhҿՔÌÀ¸ln¿æwóÂî¿ìNwÇ·º¿ïÿþÐñ?íì|*	üUNASNone4?¦'3¿V3í?³¥+:ö‰?‰<e—üŽñ?™…öLîˆ?î1û-ïbµ?¶Uß¼óε?¿	ÛNxg?»RX× |'?Ⱦ¹DkÑ?»Kþ͋º?åï0Ÿ…ÿ?ÀTÝ1Éћ?ÅÂOZÜœ?±.EŽò¥
?¿ê]‰üv?©Ú>Lß?殎Þ!*j?´‡¼$…†Â?†b*QÐ<?u]¤E! Ò?¹[¡Ä{é‡?¡Ð¹˜ýþ?ì{¶AÎ?£š¬œ´3×?œ8Ú¯<ß?·P	՚:y?"~ªÎL?¥ˆÛ²?îzIXèá?ºàzºÂob? sqìËR¡?¥M`ݚ¸C?Ìj·'íœÀ?ÂÉæ'L¡¢?çÞüÊZF?ÂÛÌYàF?½¤\*Î4×?©VO.•?¼£/¯ðóô?ª«ç…!÷Ó?è·"ª‡?³WƒÎ¸?dEF4ZŽ6?WÚºmóý)?¿‰Ÿ;0©?­h,"Q"î?ëú†ÒJBÍ?­ÖÈ©OTHER4FGL J1827.2+4303¿Þô¥Œt¡@6RÿŸ‡ð$À;$;ž;¿ÊÀ< j0'|@áH—žl½@aÙ¿#–Þ?Ñ
#hú?ÇTÒª²E¸?ôu"‡!œ?û[Õ@Ž»o?ãìá•0Ô¿êi‡]æJ¿Ç9`¿Û/dý/Á¿ì=#vý_¿ïÿŽ@)çUNASNone?îà'ü?•±†iQÓ?"¾K§3»7?{EUã¨?™ŸÈZç?'Ü"OÛ_?îÜٟ:À?˜O[u9	?…Xp\Š?'ZÝ5k—â?™¸"h¼ó?"1fÕL"B?îoùL)Î?–Ú.È÷÷?‹"ú%<?†6‰PŒ?¢iÀ¢—Ñ?'è«ûpú?íŽ4n¼t?…xY¡ê"?"×dUjÇ?rý@óé-ð?¬±ïC«b?Ð·åujY?í-Œ¤#ò_?ª/‰­Ù»Ÿ?–‰ëÉ¿d?ŠP•ÆZª·?°ñîV/?¦ã*DV?í+Çó¸ä?®c‰ú*®?š3g$k3?Ÿæ¿­£"x?°ÐÔæ+*—?¦Qž#I½?ìæá֟3Œ?¤"•`óâ?•ÎÖPÿØÛ?¦‡aàO?³U;·4`å?¡›€lË?éÝ$>´×Ê? MaÃЋ?¥.)˜†^?Ï°²ÿ¶?Ã?䞝?,p^RiÜAGN4FGL J1827.5+1141¿ïß¹ÓJë@%ô‡ü¹$À9ȄÚ`3À;÷é"mé@@ö¥8^@+¢õÚ?¼±4u¶?ÖÒóW{@v!`¢Ø@Š¥ÜÈîF?ïøTÛ#§¥¿Ø*¬¼aË¿Ü¿+Žúg¿áÑýžPãr¿íê¬"¢º¿ïÿ¶>@£UNASNone3FGL J1827.7+1141?ÄY]y?¸(Q™—ïŠ?æéòР¢?Âçñ…,¿?¿þ6Àöº?³J`Qfs?ÕeLÏ«=J?ÆhÅö2»ƒ?ÝOkü0X?Ŗëõ&á?ʖŽhIP½?Á7T––?ÉÕM™?°£;}Tø?ãÍ&L
?´ÆŒ§ÿÊ?Ƕ¾óÀE?¬'"ú=ä¶?áæÖMÔõ?£¯'
–ì?Ʉ™·÷}¥?ŸwâÖ®l?Îà
´®?œÂ6S §Z?²tÉ¡ÝA?©k²/Üt\?éæHecJí?»÷"*g?¾Xó»gäZ?³iò¬Ã2"?ÇÚa=7?ÁHÿOxZ§?âsÂÈ&C?ȱÁÝÊ9ä?Ï"€£˜:?ĎÕÌ%?¶ML4¥¾?¨\¬Ò|&Q?è!Áu¡V?´`BeJ•?ÄR9†'‰?¬ÏÕb¾'?Ñà"{5'˜?¤	Ó­*‰Û?Լ˯¸·9?­Ù–ƒƒ?Ùb¯Õ·/?©<—0ÄÕMIXED4FGL J1828.1-1312?î'(LWúñ¿íƒîÓTPÀ7酵·'À9s7+æ7Ø@"ž >¤V@mPes!?É!Þ!3ˆ?Ðå%ßÀX?þxøŠ.Ã?úaÂgÄ
¿ápÈà.(‡¿êé/~¿Ä¿åÝÐ?ÈíÅ¿é'9@=‡Ë¿íçÀn¹¿ïÿîbHÊtUNASNone?~g.æZ?Å)ĺN¯?cŒÙ°Ëh?n—ªdð«?ﯤÈCG ?…ìù~`Í?·Œ´?ˆb?¹Þ»ÞN:²?½G‡WLÃ?¶£xZ»ª"?ée‡§1e[?¿‰™Fbí?ÁtÊÇA¦?ª$¿O+y?Ä#$â&?ªlòûc
?æš8L;†®?±.›pt·V?‹lå_?uÕt¥¿"Ý?¤Ö',?Žf‡"½|õ?îRúºW˜?'mI¹ÅN¢?tn5ë'a?u ¿>.?bwóñ[z?l‰é>B¾ë?ïÄ«5x\Þ?çÇ]wÙ?¤Tƒ ¬G?©Ï¦¯?¶Z<ê?À–=¢ÍË?ê
!@—tÑ?À¸ÌWåwÇ?»Æ¦ö'‡?¤˜«¥8Gë?ÂÒäR´Ù?ªt—‰?çÒr?°…<S`?p†è¨éä?aÃbaê@Ô?©(ÌƐ?™õ†¥,<"?îLpA©D?šÌëª6¶OTHER4FGL J1828.2-3252?ⓄM›ØþÀ#˶ˆ½©CÀ;)mã2iàÀ<¬ÝpÜ@ûàÖÄó:?ú®!ÛòÚ?ÕØá-,?å'Á)h¯@
`9[k`¡@Kº5›mY¿ïߕÇ}³?ïÿ;F',¿ÊŒbN~¾¿×<(¿íwi¢ò‰¿Óã~T™µHUNASNone?ëÔ1fï4?µ'ÇôÒ£œ?¢3ÈôýR?£z·Ç¦?¸DOY^µ?°Ñ	`Ӊ½?é¡låí–W?îH}©Ï?"ô°ïáÊ?˜LmwïÔ"?Æû¶H•´Ì?ÂQf˜×?ì%ºØ6@?¤ÍèþøK?£Ÿ8ý½ÿ?"ú6_á³?µ¯5©ƒg@? q"‡2r?íÛoÚOä'?…:‰YÊ;?˜Ltú];¶?wàEÈ/²â?¦"Çߊç?€ '¹ßö?çjÒ'G?Àž—7ó?³uáHMÚP?ªSAX€mÐ?șÇ@4½;?¼F/í·Ä?äËñí1‹?Ì#ó\%T?¦¬å7
¨?°J«œf؛?Ӓ~»Fè?Êo^QïáÐ?è	'3"øß?±›¶•­ð¡?±€VYaw?ŸñS\ üË?ÇŒ"ã"Ê?­ê˜kšx?ëžÎ¨!Ð=?›"R`""?£b̵'!?¤´e0?¹X‰Yrœ‡?—Åù¬8AGN4FGL J1829.6-2545?Ô9rINÀ"`št‹À:unF.¸zÀ<HåC¼s@ÓÜäòÞ@OC427?Ó-&ÿž0W?ïþ
hø@!G'R?ìђ&ç( ?m¿Ýß<;±'¿ád¢A¿îqkGv·¿ïúYbqå ?ïå«@
11UNASNone?Ƙ"5?̐Ӟz^?Ý{ãÙ·I‹?Ðiï°°8?Ñ탡4Á?ɬÃ?ãÎO?ÂY!oçD?ÅB—¡"1G?ÛÅøÁ·Ú?ÎÜ~¬¿w`?Û
}­'"?Dz{Á	å?ÚSO@b¤C?²ówÀݪ?ÑE=€'á
?°žØˆ¯Ëç?Ôgs?z³?²1)A¨?¯)VJñ](?"±&%‹,?êH3Â>?§Ýëbw	?¾*"<m2?¢].á?Æ̓ù¾ê®?Í?d†'?Úçþfwr?ÐÕ¼Þ*v?Ù±·èº7?ÏÆ8SX—œ?ªJÛ¥À‰ì?µÛì—-Þ©?àÈü®ÅXm?Ðð°>5ù?Û$«-ô7¨?ΧÐÇ¿X?ÏÒ£4'ÆÖ?¯Ö¨òìµå?ׄ¢ù·?µKûáJMÐ?ؒl‰?µ'yÜ{E»?…_ðå⛷?uÁ.Ïok'?ë½Ha‡s@?¯\hÌM¾?¿i¾×ãù‡?­êÔÀNH¿MIXED4FGL J1829.6-4310?îíÅãÀ-Ǽ"ŽÀ;>@ÈG,À<Ñý¾Ý @zú*O	@Ôj»_¼ÿ?ÔãÌ"'áÇ?ëÊÝßCÈ@	œ?,eº?ÿSƒþ&áì?ë©È»ÆL¿ã‹¯Rhƒ¿Ä¼=Þ\í¿èwsÔãòƒ¿ïÿþÞ÷¿ìÌòÂ)ۜUNASNone?ì÷z]Y3?½WXb?§
—èö?´˜wU	?©pJéþÎâ?±ÿ÷_+z?æ˜|Bh&Ò?ÍL+PµO?ÇaC¥#îû?ÆxÜI'Í?¼y–¢vëw?½àj/ì?é¦Z›	¹Æ?®eŠ°^e?¹ñ<::Zç?¨«ÓŽû	?¸Ûîì-üm?¢c$¤rÈ?äb*\þfU?¬»ª±1?Ð k"/j?¨YÝBÆ-?¼lþ
À®?ž]ă˜?ëNž'8?½~þýe_Å?³Ù×7¹ô'?¶D¿_—c?±±47a†?±N>ò"û?ßô¶ÿ"©?ÑZ~ŒßH?ÕQ½£uKÃ?Ϲµ-s֑?Ås"?)?Á̽?çÌÙÀƒÇ?´•ó¸éu?Á¢*—Ñ?¯Ù·÷ë˜ò?Âé*ÓY?ª‹´«M3*?Ön!Ì¢r?²±ìž9ÁŒ?ÛŠÓqñN?¶-_Ï<vz?ͦÁ؁?±¶³?cìYMIXED4FGL J1830.0-1515c¿ÔÁ,íÁ0"Àc÷¦•*ŸÀ:IVH1ŒÀ;Û¸øÚr@"k³bmˆo?ÿXß_vˆ?Ÿˆ¨}®-¿¸;øÿ…±°?ñ>Õ'å!@Þø4Y£à¿âž%"ôÆç?î{P}ñÈZ¿é|í'hr°¿àòG°˜¹ ¿ÔɎÿ·°±¿àz 9påUNASNone"?Ì韡í¯?Ä_^)«õè?e†sÔ?a½ÖžŠ€?è°!É1?Äp«tô"Þ?Þ¼ü—U?͐_;ØPí?|m,§sŽý?†óy$}9œ?àh§[¥??Í=l?Ô?äø/žu˜Ö?²ÉãÁ¾£?Šˆ4[@1b?†N &D›?Õ;_ :ÌÉ?²8£­?èHí
è?¨»êl¨?'Ñ£7[m°?qP"x?Ç?Ͳf9Œê?©	f¢tª9?½‰@ŠM?¸½ÙhŸMN?vŽSÖóíz?qÀöR•å?ì!»Gzy)?¹+Z÷/gp?ÐÊ_¹gÙó?ǽÞ
xÜ?yB-}Ô§?Uš7åy¶?çhKêþÕÍ?ǖïn?Ú)<¤‡E?µÊØ+gÇ@?"_ëàÔº¯?‡ôށ³‰?âPxù(?µæ£ẏž?Ý|2¾Ì·‡?¶Üºt%Xä?›`èM0àH?"/ϓ‹˜?àfß^0:?·î½æÄ´MIXED4FGL J1830.1-0212c¿ï 
èÌ@
×õfI
À9?|–S"üÀ:́I@»²@Uñ3^|7@]gº#}?Êu¶e':Ø?áPVY¨èÂ@¥Õo2½Â?üLH=0?îˆ@
²
ª¿°†òÍèU¿¿äF­czù›¿é³©Xb˜¿íÙä"rÁ?ÐyM>!MØUNASNone3FGL J1829.9-0203c,?ªbá)XÇu?£PŒÖ"à?ÓIøBW¤"?Æ¡u'–¿A?ä´ÕÌ>¡??Æêôôç?ÇԑšÐ.?ÂË=4D«?Ô䌘:…?ÇÅyFgî?ߒ‰å2
?ÃàA'ÎÁ?ÈTá©È«?ªÛÍgC´t?ÊAâ y¥¼?¯3Éq}º¤?ãZO0·$f?²Â XÁ?¨wêrO(?"}6~ŗt?Ñ·­.)'§?¤%½"£?å¢1êD:?¤ì"vg}w?ž•'"ï–æ?'8É¥c?ÌwEmÈî?Âèæ•ñ?çí'³Mí?Ãlc>?««¬‡+.·?°º}	@¢?Ûf//©¢?ÌÑyk$?à'-ŸÓøï?ÊCÌP®¡Ç?¹çy1«Yò? 'ª*?×w?Î's}aeÝ?³­Ô
Xº?å93úr;K?´Ðl²üY<?ƒ÷;#Ú2?h¼n"ª?Ô¹»gõ‡¬?¯s' ߧ#?åVÖo,!?¯u\ääOTHER4FGL J1830.1-1440?Èe*`?Ÿ—ÀWµäRûPÀ:%ý®(`À;Y.Œ…¡@!a÷q'á@èû"°ý?®_+‰›Ÿ®¿¹%ya?ñK&õ7O"@)$衦?îçYޘ§¿â{ê'Ù±¸¿àÒZu—[Ò¿âðóˆ"xÑ¿åIׄ¶³†¿Ð?"$ghoUNASNone?ÝXM­÷Ž[?Ä ¹á3¹?nV"|â?`Kî*/Ë?á5¾Ó1bE?ı¥Ìéä?ÚÓ5>½?ÇTßa«?ˆ.ѐ:4?åâ@©×?â5ªè†?ÇSüÅ?â㇉»o?³‡ž{àÞî?F·¸?ƒ¦³·•Á'?ÙO"7øa?³^&Õ@‰"?àrù +³Q?«2è«<¾©?'0}Íëm½?wü_1éT?Þâ[ï?«[4nœ•Í?ÑýæÓ¼³®?À½¡ºê?ƒ{‡ôJQ?tv`cÕØÞ?æ´ò¨ ?Àìd=}u2?Ê~ó4.t¡?Á>£ÿ¤"?ƒ±bäªÒ»?·
œ$ß?é}§†ÓU?Á7Lï=?×ñaodD?µ<ÉFöؑ?"lÉ́6?"Ï®Š‰´´?ãkèùÔî?µIÒÁÍM"?Ë£, ´?¬>à­­·Y?Ÿ/X!h?ä|®á±4?身è?­ü`²I=MIXED4FGL J1830.3-1601¿ê{½¿ØaoÀ¥Ûüëx‰À;;?´JõÈÀ<«Ü'<®@&~Ç!' ÿ?ò(IDíoÛ?Ôπ0fû?ÂÏôŸy­k?æÒÎn|@Š'‰)ßÍ¿Ì[/ürù¿ïúÙ_­9µ?ïò×ùP¹V¿ë¤šéû±½?åg*¡iFÁ?ÎUå]gUNASNone?Þã³Tfñ?β3$ß?hD¹Ôë?'Žu'6%?àÝÊoýi?θÑ5o×?ǢlO£E?Í:žŒr•?Š"_'»Ú?—ë{&Qñ?éäUfR´?ÌÖ¡™ºž?år7
™Ø?´êÙT?|ï¢S>Mé?}£m‰Ä…?Ô§ÓZÒÖÉ?³÷Éý±éi?â5(MH˜?¿Ó…®‡à?Dk§¦j0?FN_5?ۋy'¢t?¿ÚƗuõG?Û|_p—±|?Ì~fÒ
é?oÑë>'¿´?p†¦ÂýP?â!þ\^G+?ÌŸ"Ò¬Ø?Ã9˜õQG¾?Æt‡ñDb?}…§k¶©Â?–¬íHIv?êöŽsˆ?Æ_:Ôxxô?ä¡jÑZ%:?±OdÆlû?ŒöÃTù¸…?‡8ÀÄņ?ÕÕtA¬ƒè?±9Bi®P?Íunìò²?ÀÀW•àt?J]¦ŠFf?X™Ùö?èœÿ¨þM?À&ëÀò'ÉMIXED4FGL J1830.7-1634¿ï«wœ¼LÀK~ƒ"×À8û6)‡¸ÇÀ;&‡¹E @P`@@̘å>³š?¸uË°4?ÍEɸÆ/¥@çtü+_)@Gx¶Ë¿Ä˜mŠ#!¿á*ÀH&¿ß'7<Ø"–¿ã‡ÄŸ×¡<¿é­Ìâh'¿ðUNASNone3FGL J1830.7-1630?Þ̖HMÃû?ċ£Ño¸Ž?¿ÏSFÆZd?±K"½?Ù?"ç†+?Á݋VùÑ?Ù6ñÖhú7?Åfь5i*?®â?~.Ôá?§:(Vö}?ávc–÷?Ä0íÚIÉ3?å…³Þ"J?²†û…'"¥?·ª¤ø«"?£Pk#û¸?ÐKY<(È?¯ªÚ§´m
?ܧÊPèó?¬D[<í²?°3a«Ôu1?…¡£9'­M?ßK]Dr¾?­í˜Ù²Ì?Å­dš<	?¸×òÀöV"?ͼùÅÿ(?ºÄ»¨¯ƒˆ?ãLì¨gñ4?À•3èSª¼?ÄÜ×`=q>?¾¦ÿ7Å?±l"')Ï?±¡VNÄ?è›7µ½«a?À©wrÓ1?Øy/ýÚÇó?³Jñ.W¶ˆ?Å\x¤µ	??ª¼õ%qÙ«?Üؓ¯Ê³m?²C©2ñ?Í^ɹòÕu?©ûõâÎI'?·DYm¦îä?›veÛþ£G?å¿ÂcÎlÆ?±g&ˆ]±MIXED4FGL J1830.7-3219¿½ÁJü:À$K-
$F0À:M)¹6íÓÀ;ï>FŒ¬K@
ovZzJ@òǝ¸ã?̱¬µÖB?КtŒB@K/©:÷M@]i·?ìŽPrß?ïùâå=¿å>f˜¿åOÍ2MZ&¿ë)˜JA¿ï…õåÊËUNASNone?ìíÚ¬¢?­§D_–.?ƒ}bЋï?|'8+át?¶'TÐäIñ?«¼%ï)£O?ë"éš|²?¾eø8OA?ˆâgNàç?a:
E‡?Áé€E8*?½"ùnY?í	Š| ?¡p×þÅs?Žª0æ?…‡óÔÎxô?³Þ±¨csÞ?Ÿ0þ‹ÇÛ?쁚Ð.Ú? áï@6ž?¡É¨àFlÅ?gæC˜gŠ?³U´´Ì?‰O'GƟ?çðÿº	üƒ?¾È*uË?›Ú­yå
$?'~:öÿƒâ?ÌÀ«i®M?½]Åí5<?ç3"]·?Èlêl£tí?žKÅ-ú—¿?¦Û(=ão¹?ÏjyIܱ¶?Ç_GËõó?éÉËy™?¯ò³"¬Û?¢Bá-Ê»?"8£Œ@þh?Ç`#‡ª¿î?¬—/þg§ï?çܕ'2Ê®?¤÷žêt$?³nÉLq—?™e–ŠÆ?ÆÖEwêƒ}?¡EWI©FAGN4FGL J1830.8-3132¿ç×#/"ýÖÀ#aE•6À:>üGä› À<f°b2úÿ@ø$ EŲ?ýÖjÛ@-?Ãöó<?áwT€	û@0tBÇû­?÷ŒÈ¨zÝí?íÇh¿‡¿Úÿ'}ž;?Ç؎÷Õ:¿â,Æœ/¿ëº5¤¿ïý¾1)UNASNone3FGL J1830.8-3136?°?½s•-a?°†Þ¯Ïñ,?éOkh;?¸¡˜Q×?¢tì]ƒ5?»àþic?±PU—†ûÏ?³}4&ÃÑ5?à¼áyÏq9?È1'Jº?Ú2'¦HdÚ?ÇB-õþí?Áhq@ëO?¨Ô~®N?æ"¶G™?²¹—8ÉÓ§?ćP
UöN?«•(dñ›?Ð*ՙ،Q?£¹b‹·ð?ÞŒèíP?°eÕÒß?Ñѝ}:#¤?§5×OΧ?Ÿ¯‰¯'‰?—·
F/Qa?éTðˆ:?¾‹‡•¦Á?ƶNlZØO?¼WÞ£¹Øÿ?¤E»ÿ¨?®å3ÃHa?áþDbŸKN?Îv™J¥|?ـ.'¹0?Í1U7"ì·?±ˆiOÊá? ÅvÐÆ»?èú~î"ë?²h›m*ç?ÃQϞ–â
?®
P¹
?ºÿF1<¸î?›îòQñ®;?àãÃ'¹œ?¹.†®7ù?×x¨Oa^Œ?µ">0WÚ´PSR4FGL J1831.1-6503¿ïíȉµå™À6YTdÜ"«À:NRå€!ùÀ<‹Å£ãŸw@$Á'|D?ýŒMryš?Àúpßf,…?ÛRº·÷R²@RîcŠ	?üܼŸ‰?~@ÈG,¿•sG R›X¿Óðe£ráI¿ã˜a‹5S¿íçJýTT¿ïþ®û*®UNASNone3FGL J1831.6-6503?¸Ð¡‡Övå?·Þ5Ä3ÖY?ë'BXÕ+?¿eRj0'?¥:—k#ƒ?¦/÷4A‹?Îõ÷»|²?ÓFh+¸?ä8Âé–~?ÄRwsKs"?À'óaê‰T?´^ò×2b?À!B3Åîü?¨ºfZn ?ç­Ãm[*Ò?±÷6Ýh¤¥?Á'°Íe¾?ª$¡ëÀ?ÜCx«Ù?©9wšC?תýÁ§?ªŒ8yls3?È#W$ÿê?ŸAÁLƒ>Î?°y·!?ªp=u?ì›ûÊ¢aP?µ ðνEy?¦6XVÁ?¥äcoÑ?Ù&aé
?ÀÃô°…];?æé㊘8µ?Å}2nì™?À¿Ksµž!?¶–)Aí¶&?®e&Üˆa?m«ŸÃŽ¼?ênt<gåB?¯9oN¡¶?½YÊÐâõÈ?ª+²]ì?Ìž Uϯ?¦ªõëâ¹4?ßS´é½Y£?²ðKžÐ?g?ҟü¾…?«Ì}=4Â>MIXED4FGL J1831.2+0202?à3eì*ê@¬óý">6À9ž;1.v5À;¡]³9@sŸ4
N@7ÜËè¡?Ê]u&Ê;?º;²!""?ïwLg·Ÿ@Ñ#rJö¿ÁŒˆy‹²%¿Ù'k\ÅRÛ¿ëÝQŸ"ë¿âKu°†E¿ä0#̎¿ì$P±*UNASNone?äcöÈHÚ?Ä܃ƒØ'(?‡m:(—d?Œ!w¯?Ö~u¹?ĝ¦†3'±?é8'ä
°?¾£1°·?ŠT^5œBa?Ž
>˜FQV?ÉzÊÙX?¼¸ªÒ<O?äïÕþyÃ?²À؎&<ã?§ÈNhç̸?˜ìÒð‹‡?Ó'J5	ª?±'•jëX?ê–WvÎ,b?£Ã^ÿˆÄ‡?x÷èKYÎ?`GùCÆNé?ď¦?£uH}-Žj?ÞüÏ,A¢?Ä$c{iF¯?'Ï.Ööÿù?0¦5ë;¦?ßæ=çl5]?Ä::Šÿ?â\‰J"¢?Ç[éX<?šäc´ˆÇà?¦©©6c¢
?٘§‰Ï՞?Ş3žàLÔ?ÝKJÔî?´ëF\9?±G9?ž'nF;š?ÞQccÁ_J?´pŠ"‰ˆ?ä3Å}o?µ5€FÌ8?"»ÿ•¹õŒ?y:[e¤:?Ö^({"K?µV×Cœ'šMIXED4FGL J1831.6-0223c¿îÛyaÚW@
orÖٖÀ8® HtäÀ:b4"F{å@~og–è@ñm*¥Åø?ÆèÐ#ˆã?ϏŠâq¤³@?òÿf}
?ù~‹=á7?ïh
?®–¬?ã"Ág	¿ã^PþJHN¿ævéki¦¿ê±ôÆ/¿ï÷™^á6çUNASNone3FGL J1831.7-0230 ?ÀèD¨âž?¿Pʦ_ƒQ?Å`fŸT¢?îQ â?æmÕU(ó·?ÎoXòUë?ÀØ´¬Åpb?½Œ¦8…ÏÛ?Õ¢\r?řꈅ±A?áF¦•¢á?ÄÙsNVO?Æj)¥¦ÿ?­'W²Äc?ÅêÆ1ýÿ?ª-‡‰·ÿT?å*Ä
À?²@ýö£Pv? Åt?Ü©?j£a?rH?Å¥
w8ã? 2_T¢O?éŠl*©)?¡ãûL?¹çßUn$)?¹þªp??Î@ÓÔ?Ê¿'‰|bt?å3fæ¥?ÑØú×eñ»?§Ù+Š/^á?­Ä«åþJi?Ù(¿sÀ8Œ?ËNh7Ý×?áî
úL?ɒáàkvW?¾)1ßm…·?£Ò†GÇ}?Å}¶0 ~2?­
jýüµ?æÛl7ê/½?±sÌi³I"?"IœßOØo?lðúÎB»¸?È1¥OÁp?§Ë*ôÖ?駍#Ô?§úäzG­OTHER4FGL J1832.4-0152c¿åý*Hð@
û–C£Ã¿À9*螺jÊÀ:ŸFŸ@èˆòWuÞ@ŽY½
·ê?Å};‡õ'?´Œ5'î²P?ñ³WN›o?í¹ž"!­?ïŸÈ‡Ã®@¿ã³Ú°¿åÓZ'És¿êYÙUm¿ØCÑ(l0¿îûž ç×UNASNone<?Ó£|F«?ÉD«!ª?–ëÜü)?›>*4ð?åw`ÙM}?ÉK73ÑqU?Úmk'9ç?Ê®äq%©?¯ëòZKÀ?°;V…WI;?àʋ҈?É$Îqù¨´?Öä€2?mS?´cv+ì?·Öü"©6ë?¤UØñ?á'àb´]É?´'í:…«ß?¸còçRYö?šµ£¾Ë'<?¡]Á³0r?†ñWT`?ëâ»Çþš?Ÿmþ¶(ñ?Å §Í0lQ?Á	WªêW€?"+ΦEîZ?"À͓…Ô!?éþw—f8™?Á"Ï…cז?Är˜Ù€9v?Á*;­je?¹Ò…;œ@ñ?¿/‹¼iÛÄ?ç©	",i"?ÄõäÉá?Ë*¸@ßÕN?®œž'é™?·×²ÍÕÝÙ?¥^ݨ^¥Ê?æ:[–(ËÑ?²Z
mŸíP?úëKƅ"?ˆÛé
Ë)?¢Oæç
w?'V@…TˆÛ?íë*6úü?—3!W£ýOTHER4FGL J1834.2-0827c¿»ß׿²\›ao܇À88+"Ù@yÀ9­¢uá-­@'£Ýë-@D@yJ?È%µœ.ŸP?ãÖ³ «Ü'@[WG9?ô'qº,Œ%¿¸ºË,Ž©?áÌ•¶¿áP‡×Ð6¿í7åžTê¿èœåžªÐy¿ïõ'àhUNASNone0?'F¤aO¤?¤4œ³×?¶qù¦á?ëž¿V?쟐(¬œ?ÆL»OKí"?¡Ðáí5ò?§'¸Êš)?Òé6‰mÁ?Á±ÅõÃ6?åFfß?Àpáxš4c?­pàaÛæf?ºÄ6¦/T?¾Ã®§Ë?¨é¿19Ñ?êP|8y‡ð?­óŠwxî?bU:Í6ü*?IÆþYíik?ÊhÐy8"?¨ã¶PI?éSvÁõ¥«?©õ[*Uæ?€¡§ž)Í4?L»…×¹É?»èîkƒ?ÅJ/ñV¼G?ìM|C·(º?Æ]òѐ£H?†ðz^½f?'kT¦p?ÔJì}AIK?ÆlaìÈÚi?å~ÇØ`²?Åçõæ)GÖ?¥ÌÝX*Õ?—uÂÑ5?½ø‹þŒž›?ªåyM-?êä ª´7ï?®
Ï×MÒ?@rdHì?0ÎU
µ?Ñ5qOè9?·Ÿ&Zd?ça*Õõ,?·$ö[³ÒLOTHER4FGL J1834.3+0613?ÚöÄË"@‰¼Ö_À:/ÞM'ÐÿÀ;èPÕ©³@,Eü
­@lKÅÑ0	?Ç·v¤L%?Ûê-/ãó@
Ew{a .?ù™²
ԚL¿äIq-iŖ¿ã»àÑn¿ßù;.ª¿â=@26ý¿ïúá¸\?Ôùr²¥ZUNASNone?рƒ¼M"?½åäF¢7?ǹÚ%6?¹—·›/?á}ßþÐ"?ÁõÆJ}?՟c Áߑ?ŌtW•¾?͌|ˆOð?Á*'Õf4¤?ۚ^\ùøv?±A´‰?Ý6¼µR‡·?³"·Drh?ÊìŽ9¥Nj?¬-` Ô¡W?ÕRü-ÚÑ?±œÁ¡ö_m?ߑ_ýxš?¨‹[ø_‰?ɬ
ò]'?£ÚkM¯J?Әsvwß?¤N' Ú¹?ÀiЏ2
?±	Cÿõ?ˑíëLáý?¾¸
3U~?å}?Šž?Àø)­|?¾JpÖE¶1?¼íLôû?&?×:/-r³?Ê&	ý¸Z­?à™±Í á?Èá]ó¦*w?Ñ- ­¹P?°Y´¢'£?ÒØp°úð?µì™}ˆû?Ûú}Ú¡KÀ?·"ì¦øK?ÇÚÀš(N˜?£­‡#žâ?Õ@M¦.°ö?³#ÌßqA?ÞÒR
Ð}?±uLLþ™MIXED4FGL J1834.7-0724c?脈 x?Óñ(̧ãßÀ8Ní·þßoÀ9ógÁLf@CÏ*J+r@7õbLM?Æ('Á—å?Ýdéc±UM@_Ɨ(¦@I¯¡mÎ?ÖÔÀdïn¿Üœž^€>¿áWàÌV¿êÁ+Xô¿éûÔÂd"þ¿ïÿß~€8 UNASNone0?ÛQDÍ+Æ?­¤F#ƒp?µ¥–ûÉS?³Tÿ?¶…U?ìĄÐâ(?´j™'å¿?¥ÙDœ?§†rÒ-Õh?ŦíÍÔE?µúÙC?éEW™U?¸#Ðx£B?©j¾aæT?™Ë#jÃaL?Ä¸,#?­ÌëÇ?é-|a>M1?°•¬±»?Š·üPàý?mDî"Èö?ÁV³|*?šiêªXX²?ëS@9+ß?›¢Ý6½±p?V®*>¨?v£
C/½?¿¶ê¸E+?¸Ú3ò¸Ø?ë×0ãøp?¹0RrÝzì?R¡Óóß@?•G—Ýñ|?ȉÅÈîé$?¼ÈÄ®´øŠ?éZùw]?¼ÈF¸«e?¤ˆù=?'Nµ¨jƒ1?ÄȂÃÇÉ
?°ÀÉã8À?éŒV¿Ì«Œ?±•øðl99?hã/Áäé[?SÊýÑéÍ}?Äæg"ìZ?¥.¹ÀšS?ꭂï€xX?¥AÉ©OTHER4FGL J1834.9-0800?×{‡MšED¿‹ò7jzr7À8²ò03¤À9§†P¹Œ@diÁºŸú@ÿ³Ä¾
'?ÃʀÂ2??Ú)åè
@XÁTɅð?úS—™åô?ïtôhó¡¿Üá‡ÚTtÌ¿å÷aËÌó¿é¤cOοïýv:ÂÊ¿ïñ`[_wUNASNone?"!fȅ4?›ý.ÂÊ»1?§B+—µA?­•óí"®?íòÒiÀÊ?²N͇K¨?¢£¥ÁX?¥>ô_ø^?ÒÏó—U¶Z?½´[¸sµ–?åmËØ[ b?»þ·ƒ÷?µ¥Ö½H?¤¸B¯°Þ?ʃ'efd?²ª<¢²Aè?æ½*«­ËÞ?´š
ƒ(Î\?hål[hö?PÝ%â"U?Æ6°'éÞ?£;ú-ãP
?êYno/žå?£uÌØ,ɯ?‡b$<"=·?¬°‰åb?´ç걃d?´;`áéªÙ?ízÜ-?¸ú¨ÖU?‡Òa¬€?ÁbáK´ß?ÔFôÍ7ú?ÃÐÁ›b¾Þ?å}<QmR?ÐH;qßÛ?ª&÷9؟Ü?€Â^?ÉiÐötˆ?´ÿDñyÔ?èöp?¶(m/"?F4OÖ`ÑH?5kÙRôg;?ÌC%	µò|?¯ûí­µ2ç?èé©©~‹n?°TSÒOTHER4FGL J1834.9-2819?눣‡ÙþÀ"m‹`ñ²_À9ß)ã(XåÀ;¡?
×ÊW@A­RÞõ@õ†"X?ƃX$.]‹?Ì¿$³h£@©/¤2yÐ@jTXœÏ.?ï([žŒG¡¿äV¢¤W¿èû$Ų&¿ä¦^ê–¿ïþ×@Än?âÇÍSÛIgUNASNone?çup¦Aƒê?ÀÍ$Yjn?˜¦"%Îw›?'Þv3>h?Ïlâ	'¥?À	24@à?çùI'ˆAò?Ã[åyA	‹?•ŸáÙC?œ†NJiD?ÍféÁØ°Ž?Â
uöbƒ"?ëÓÚñِ?¤G¿ ¾·?–#òíUªî?†Ü^á?»Ø2¾e£??¢+C9`å?ëê½Ñ?"Þ¤¡ÆŸó?š—Ž4]@?x䶷n¥?ºñyCQ¨?'ÍÁP¨ö?àãK`Èå?ÄüÕ¦îŸc?¨_ƒÉþ°,? ÍrRò…?Û-xÅIÜÔ?Ä~¡cƳ?àÈÂÓ­?˸8\#'´?ª(Ð	˜?°-?wll?Û-ÎÛÖç?Ë8}n"†Ò?å56{CI?²°/Ë?®·œ9L¡?š'¹ÎÛTV?Ѿ²6I™?°×$.?ä¢psÁ©ê?©tèû–4?²Ú>Åû†Ð?•í­?Î?ҏfÖø?¦ŽÞbrý(AGN4FGL J1835.1-0517?Õ}5‹ä5…?óÄÀ:9tãë¸À;àæ½2%@¡ŸËŒÜ@N$PAa?ÔØèd?ïö?!}ÿ	@я1a@[î\>šE¿îäÍ_ê2?ï}ì?õ(?ØCôáé¿w¿éÍî \+z¿ìTÙÁQïa¿ï‹6môOUNASNone?®	ãR§#?¢ó€x‡çp?¾å%ð:Ì@?²¼ü6ê[?êB½÷pv?¶þrõå?©Ë‡Îýð?³ŸûM½?×9¥š¦+p?ÇÍØ8
Á?âÆt¶щ?Çúz9×è	?Ô¤Owêr?±!¶®\L?ÎkRôčŽ?¯I¯Ïc;?Ü&g8¯…?²­$½ñßù?Ê«
ïE·^?¦GB Îr?àC¼ðX9Ÿ?³ m¸*ò?Ò"ÿ'¬±?®ž¹ë¢?¡-mí‹â?™2¼'Xaà?ÂâsŠÍ¡?¶¶ãÛ2ö_?ê4Œ>'6ú?¸ÃØ®€§?Ÿ¤¹™zv$?¥ö5kª"?ڋ²t½?Θlu£"?á½'>Õ ?ÎiüÀQá–?ǎpàV±+?¨e–Æë?Ó¤rÕNj`?µ¦¡Àcñ?àJ*]C…?¶mM£É^³?µ;Î	?žÛî3ìïí?âMnÝ¥¯?º¨[‹8z<?Ö?%Û?¸8šŸTÎÌMIXED4FGL J1835.3-2439¿îaR;ÚÜÀµK 'ßÀ9¿WeA£8À;]Û8 Z~@2۞ ç×@‹@š?Ä2·¸=Ÿ?®h²ñÚMi?êHQY•?ýŽücé4?ïñ"aÔ±H¿çMž§öT¿ër4€:M¿àõÓ÷cyL¿êm)™V}»¿ÛVÂd>UNASNone?ᰏn6X?Ã
sèÒ^?†|8Â|"?yàf¢mH?Ý:½!fj?Ã¥ÇzR'?äŸÿÙáՕ?³ßÿ75Õ?Œ,%¯"¶?ŒӆOdí?Õޟ'×Þy?Â:2¡ì?äÂûž'»?±&œd~?¢·,½ÓS²?"Ú%B2>?Ô##*Òf•?°¾$W'½?ç©_?¤eü‡p9?Ÿ6"i1z?y4šEÎÜÁ?Ð
¤"¹$?£1âÿ}Éæ?Ññ
Ž¬ß?À9¡Pб?"J~ê›Þ¦?‹p'Ae?æm)ë?À¤6ئ—%?ÕÓ'Ö÷?Ätq"úM[?˜j'Wo?£xi{Í3ƒ?äS bœé?ÄÁc³¿Æ»?ÜÐÍd™ª?²}öš?«¶í\LL®?™•8ºu?߸TïŠUÉ?²ÑÕ9ÄF?ÚÓUö_Jò?®ƒÿ<V_˜?²G¿ÎøÑ,?" 1lp ?àM]
È?°#©‡H?QMIXED4FGL J1836.8-2354¿ëè×'™¢À"?ãDÞVÀ:BžHUÀ;¯ô"q<@
BTä2ð@ä¼B;
ó?Çè-%}$?Þç	úTÅT@*ܾ²W×@ôòÌæ£
?î)Xb—¥¿Ù¤›À»F"¿à]/…ÿ‰¿éÅ>=}d¿ïúȈšmÕ¿ïü™^
wRUNASNone3FGL J1837.3-2403?ËÀQg.k?¸fY#:uO?ÄlҞtù?·=ŠÎE_ë?ãô¶þ¯H?Á
@"̃¯?Ö:Àk‡&?Æ|ÛƘ]ã?ľßø_Õ?¼`̧·?ßeÏsh1?ŵ#."y?Û†Ùª?³.ô¬‡)w?ÊZ¯#³Ö?­æIÖ¥Î?×¹"R‡®­?²jû±Z¹1?ÙÏc"hÇ?¡M>iu¤?Êt!žúñ<?œúQH9®?Øö‹œÀ_?¡|\H¾%?¶S!u­"?¨Jô²ÿM?ÅïßÌXß?¸`y®RõW?çîÙAØÆ?¼8æ"›?Å: ùÀ?Á4äeg/\?ÏÈ¡Dí?ŌÛàÌ?âïe™óí´?ÉgÜÙÆk›?Ë?(th\¶?­ô0õ…r?ÑoÕ'm{?´~jëÐ+?àxKZ"Á¶?µ¤.Tôpw?ÃtAõ‡šØ?š
'ìF?Òõ—ºNùk?ª[B욺¯?á¨#¥vœ"?ª£o²õžMIXED4FGL J1836.9+4439¿Ûå Ë3'õ@5!S‰Ò|À;
»DåÀ<Ì&Tþ_@ ìw‹§¾u?ý7†ª×¯?ÒQ/|}?Í|õžþ'?ö5…£BÈ@AÊ¢ûíø?ïÿn?x»Ô¿ïÿ"~LŒ ?ïó˧nn¿âº‰ yÞ¿ß:i]f¸q¿ÖÏo~èé8UNASNone?ïtlÝè—È?™[½ª•ÌM?J^m
$à?@ò]ÒÊÕM?Ÿp،ø?™F-ø|?ïEPÒ*"¹?"Eêxš¾?sÃc‹xk7?x—[¾"(4?'eÜø¸?˜O$|øS?îfu›É°Ê?œ'µÈñ˜V?oàŽG™?rê‰½­Ç?§§E³ü6ì?›Ô8eœóÞ?î°ÃÙLü¢?"‹fuŽ?gãDò`û?Y˜'ÓŒ•?£uŠt!_Ø?ƒoè¡»»P?î›MiÑf ?¦Åw3"Y?[0Pu?Sç|þd¾«?¥q¨À§EA?¦¤0Ù3.ù?îS…ô¡'?§Éþ؋èn?€8/hÇ¡?‹¿Æ¦ƒg?¦¸ëÄ^¿(?¥Ñ̈́Ü?íT4&'n?¡â¢_Üv?z`sèÛ?{â%¥Dâ?³¸WŠUƒë?¡•ðT¬Î¬?ì$b4tô?£õØçe¾ñ?vGwÒӔ?rÖ5\}aY?½xvìÛ?£¸Ôµ™AGN4FGL J1837.9-0620?ê,L>œóÁ?¸Þm^'RªÀ8œá8"œÀ9ÔQžXE@äq–ñº@…à1?Ím6d@y?Ò¹–å	Y›@Ùs¤<ŠË@#ûó+g¿éMóÉøÝ?Ùä¼Îa¿åvÿ:Þ"`¿Ö=9T¿ëÍ/(·Ä¿ä?©þk«UNASNone?¡f´­ÛÀ½?›¹'˜ GÉ?¦¦EW*¼Ë?¤Íaíè?í0_¡Ù¸?«ç£¥§"?²"dÖ?³¼Ôgbõ?»8ԇ×$j?µÿÓ2¸&1?êFe"ª¶?»ÕÖ%ªÎ?½µm"4?¥k—Y¡§?É:	;=ã?°2XÐx>Z?æ§~S‡?±¢ìë°z¢?£Cw(I'ý?ŒVÇ»?©Ç,ã*?'ÄUxæ?í:Lƒán?šªP*w¾L?•xMòæ¸?Žº)®ë‰?«·kb_×½?¨ëÄÝà³?훥‡…è.?«eÚ/£ì
?¡¯/[vï?£¼'Ôôш?ƖØÐwbs?Ś9¥pÅî?é?VÖa²3?Åi¹y'o?¸û\#¹ºï?¡Cµäcè?Ì™ $£#?±6S]9ó?åÛîŸÚ?±äܜ7SŠ?‡	†{)£?x2)ØÖm?°k+\ªD?ŸÙiGª)-?í–eÔ_1?¡[¹œëÉíOTHER4FGL J1838.1-3352?ão4òbÀ(f¨ü
,8À:·?Úáb†À<˜úà@*¬C•V@茊½^?ÔzD¿¢˜?×c0œ*¬@|íáðJ€@u+ùX?ïÿÏ"èbU¿êƒÙ©T!À¿ÛÆ\Õn¿æÈl뻥]¿çžôí}F}¿ïü¥'†·UNASNone?îÿîåÑUž?–"ì]L<?`ÇíRd?X¨áO¡ú?é?ãß|Â?•v"5Ù?뎵î?À=q«ûO?‹—ÁÇÿ?'FôcÈ/?ÁîŠ0^ÜH?¾¥#Ä
Ä?íLmb?K? zŸˆÌ?"PB>',«?‹{"©}'Ü?°È"_<ÿÏ?œ™Œ_ñÄ?ìMÝ®‹?Œ–š"åäõ?'ÅÅ÷|?lGM™S_?»X¦V¸ÀÉ?ŠöÕ |?íšJåÙþ?¨µ¾y‰"?t¢Ðv8å$?s²=ˆVe?±ã'RÍy½?¨)òƒï?æÙ¢mJ'¹?ɤ¬¥Ã|?ž†îÇ‹V?§`AZԒ?ÐdL8pgz?Ȋİ"ÓË?êØ9mñw?¨£uBOÅ`?¢9nÀåÔ?•h!ãÄÅ?ÀKî"ë?¤êjç[l®?æ
…í•DJ?£-ÌÝaò?ŸûèV0²Q?‡©ˆù.Î?Ñë5ŸxÇ?¢Às×uï²AGN4FGL J1838.2+3223?'¿d¨wã#@0´£ø˜,²À::Å%8ž­À<Ñ%÷áN@°ZŒ¾iÞ@^P?³t6?Åòw×'É?Ðÿ ß‰@ºVwÜ?üºËÃbk¿áòýž%ðU¿Ñ	£ðÝM¿â͇<ŸÃ¿ê7‡UÊ6ð¿é5:ßÏÞпïÿöùŠpUNASNone?ìÒÛ¸*±ã?±¸ÄÂnE?žüUWs¥?"ÒW .eò?±ãc'œÆ?°'q(‹?êñ¢%­?ºM´O
Àn?µ×b"—¶?²|0lÎB??²›ŒCŸÛá?¬.¥€"Ê^?ëÎ8Gê?¨
8=WP(?«*ÅV"ó¥?šÚfš<!†?º,+Žñla?¢m¶P"]å?çҜ˜ã¢b?™b z¢î?¸›¥ôï÷6?';ÇC{?Ägº 
³?•×{+¹O?枔ËÝO?¼ôGá§5 ?»Ñ'ÌS‰?°ê#ÖNÕ?ǝ!%}?¸s‹›Å{?ä=Š€ˆ6×?Çޅ¥¾?ÌAŸ²?č&ñ¨Æ«?Ã	»¼?r?µÝ*¨ã"?åX–"#Ë?²öSÖþ?¾½ì…àæE?§å ­Yöß?Ë>¯n©<5?®8¯Ìpbg?ÝÔDžìp?¦f6±ƒ?É@k'ôÄ@?§…ƒü¾ò?ՋæAñp?©GÕFañßAGN4FGL J1838.4-0630c?ëΐ=Ç®!¿¶5U"…XÀ8ÖòJ¶ÝÀ9ßL¤@!7væfPí@ÙÒmrÊ?âh°ºG?¶'à~ÀÃ?òÈ4L7æ÷@—IEbø?æí½¨l›4¿ë,$ˆþA¿â*Œ 	_пéÇô@.C_¿êf££׿©½ï¦ìhUNASNone8?›
ÄxA9™?˜PÇm½GÊ?d¶EÉNB? ÖØUÇ?îâI-?¥C~_'ú?²Æ_g/]?ºhݱmî?›W/Ci?£=}÷ý?ìÌ|	]CI?¼d¥Ï2?½anH̼K?¦\AëÏõ¶?·
 |ŒÃr?¤‹^è?ér'TÐ?­[Ž÷;!?§;Ÿ%e8k?ŒÚÕnÉò?y¯ªùx‡g?mÉý¼8<ù?îX淕¿+?Žq:
V%?'ÏwßÑ—?•A/¤-?FRiGæ?£È‰ƒ7\­?ï2÷œVL?¦¶A®Á¶ÿ?¨:ڗFË?­˜º˜Äé?›Oty§öO?§¦6%¥â?í¤®—
Q?³T>†þ€\?¶åòÙ«÷M?¡`
¸²è?µ¯Ábn0Ë?£‰m©0"x?êmIx³´½?ªj!ëcðþ?ŠfŽ‹eÒ¬?x'^Ub•q?q>¹žNº?uA)…%i?ïtYH›¥8?ޜq|ýQOTHER4FGL J1838.4-0545?פ¦YÞ]?Ïþçüþî³À8Pª<À9LWšÈÙ@#ì°	‡@1ó:ß¿?͖9'ÈÅ?Ù²…"êÔ@<¬Ñ"Âr?ôªm9>e?ƦÊYªì'¿ÓÁ*¡OÆ¿ä€þ "o¿ç¸ˆb½Þ¿îxIRYi(¿ïä$7í'UNASNone?qžµx'L?uZ±º=L=?"z´èYº? [›9àT?ï@î%s=K?¡ÉÆ÷•2?§ÈYÁ)?¦HËD¿?Æ0Ê¡˜?º9æ£é?醏(¨?º¹•«N?°-ôs[¡¤?œ"z6K`?ÄOÜ>ãHB?¬p\°m6?èæJaÍûK?®Ò&z~{z?\åbÿÙ[}?Iµ'öë?±K˜m•FÞ?—춁è‡?íÈ@щþ?˜l8§?eE¡ƒ ™u?d=ñœÓ6?'£`H¾U~?›çt¨Oh>?ïUŸ[ûSs?-?yè?‹i3èhHd?•`æçق8?ÉÐSñTýš?ÁÀŽù¶‡?éF4Ýè?Áw³9l¢?¨JۆÔ?"ƒVuÓLá?ÅeŽ3MÏ?°ô§0€ÝR?é!î»Áý?± Íq`¶?=ÕG&£²?2	/U^	?´É"1I?¢"¢U¯,?ícV….?¢5(SKАOTHER4FGL J1838.5+3837¿ÂÔ
­V~¬@2áô™=SÀ:µÌ÷"÷sÀ<[]À¥w@"?6¡§°@Æñ'9y?ņ¢Ücm¹?ƒd·î!
õ?¼öxýí@õýÁ¿Îeô{'r‰¿ë]BÑ5è¿ãù½@gÏ¿â?õž}.)¿ïý'ÞZ"¿ê;Ì^èãUNASNone3FGL J1838.1+3827?ï—Ur´c±?¦DÐkG3·?mg/ú?®&w¾·?'Ðâ…l£.?œìQÍR-Ê?﬩ë¯Ù?'Åܱ?_•nþ™°?eès1Öè?€ãrt6ž?z§sCeý­?ï¹•S~?‰}ñf­´?zê¼J–J³?{Y#³˜Ä?•N/Vèk¥?":"»Ê'?ïƒYª||?g7œ÷³²?l"¨åü'?PNÙA†ú?ˆ«û}?cd©&oJz?îÒgQ•@?ªÄ2	9?'µÁ>"J?‡ÓçÕ.´?œaòqºÖ?¦g+¥xµ?ï
2n£\ø?F';C"?u
¿•çfa?ˆŒý«œ8v?™@›'n?•ÿâïfY?î3`ó"h±?•—c»9?‡½K'Š²?ƒ°q`	;þ?¦Úâ&ñÉ?' ¤ýZF8?·†z¿?†ìŸÜñá?"_/Ìå	?q"5ÒÒLÍ? þ ½ðJ?'dñkNJ'AGN4FGL J1838.7-0601?áL8±–?°uÙöÖáyÀ8öþ	…»À9ýtšÜ¸@"Ž3ºí|E@ir¥9

?ÏufI
5
?µú¥D"?ðŠ"˜±<N@֛öEŒ¿Ý(âø2V¿ÀQ°â5"·?ͳb(¤9¿ß¼¤`œøÊ¿æ{ï?z¿á©ø!mUNASNone?Dk¢Œóž?†D+¨û6m?ZÖí;ôú?_€wn'y6?ïu'ÚÕ?‡hßÒ?³°Å9÷?ºE£k]#Ð?–I·G}¹?ž 6M¼BÞ?ìë"6X#?»Ò™*F?¾ê#¨YY?¦Isƒ³½Ø?²?EÂÛF?¤]xDç?éè4?®%#·%Ö?­3GLޟ?'ÿ†íÌJ?yýñ,¡?eèx¨öíQ?íøч
•?'ÈÇM"¯æ?ºÙ'H•°?'$‡p
¢Æ?b²ûyåGŽ?Ÿ¹ŽZ
w?ïvažU–
? Z¦"©Å·?«¦!†EP'?¯ÙÄo'&?")ÐøšIÝ?¤‡m¡?í¤O_ä—?³‰¾<>ã?µã''w-·?¡;']PŒ?®Cº\5I´?¢VCô?ë__h	BŽ?ª'ÈùfZh?"l'$…Ez?'!𠨊Û?wlÎEVü?mŒ	Ê?e?ï-ÁÒíÌ?"ä—ùï5OTHER4FGL J1839.0-1502?èø×0˜À‡zA¾	À9–ä+Ž#À;4Á5¿Õ@Ÿ?´öÂ?@›:Æ¥k_?ÉCáè<ë?ÓKaþ!Ùo@ÊôW@eÜRÑ´?ïÿHë+\¥¿Ý2/'"š¿é(¯ Ä¿â7wÀÖÊR¿ï®+ALP'¿ïÿø]ˆòUNASNone?ÚcŠÓFþ0?Äm)AJ€µ?‹tõ¥}
i?'3SöÁw¸?â`f¿t?Äs¢wlP¿?áO³'ùÝì? ¤ä'Û? j…y¹ðË?›{Ÿ±×@?ÛSI'o?Á«6¯¿uÌ?ã,ŽÈýÃ?°¦örý<p?µªÌe˾?¡\K!¿×í?Ô</eô%¬?®uøÝOe"?ááي†'g?§Ä–VõÙV?±žRŠ€:è?Œ€",JËP?×Ô¸HÜ<×?¨(Ÿü6;?Æï¯c8G?¹w-דJ+?œ{ÛR'"c?›L^Õ~?é`5L"£?»`U!¼à"?ЫöæM:?ÁsTuÎ
?©¶‰ÚØÖ?ªd©ˆ?æ)$*p†?Âk
âc.?Õ\'Œ[?°lÏs0©_?À(Z;)Þ?¦¥­áë'?áG ó«?±Y9ÐWÝ?Ӄ݄í¦?«Yaíœ*b?¼O4ô­Î? ;Y	–½?â´*½Ôós?°¹ÿjUuMIXED4FGL J1840.4-1705¿ç±€x‹WÀ]^^Z(kÀ:NH;Øô"À;¸©Þ‹;2@ ‰iw½Ñ²@½D™?ÒYª–A ?Ì'—ÉŠÍú?üö¡ÍDÁÑ@xœHöi?ïíTa$X¿îL'\f2?Ùþb;^zà¿å°ý-½¨m¿ìêÛ@-¹?Ä=må™!UNASNone?ÒgELC<?Á1w5/{‡?'­B8!?‡6ªR&þ?æ8_ñ"fá?ÁÁ¬6™?áÙ²Ÿ‹?Äéí.—3?'¿;Œ˜5?"æ¹±1ÓÇ?ܝæ"P?Ä!y'*N!?åŸK‰¸b?°) 'ƒJÏ?¨g‡FÝi?—O¹Z·?ѯ[úʏ?­ÖG2º)—?ââzªQ]ý?«šÏÖjÐñ?¢³jU>ÿ?Œ†ÅŠö•?×ägÉ+Ç?«ÅÌ­Œ"Š?Ä>¨x?èß?¶ïȝ¡P? {#÷Påé?˜ºnñèI²?é裢±ñ)?¹÷y¢òøt?ϗCw'Íf?Áæ­¿ä?˜Ç'ÊN_?¡u–íÞ9?çSò"äVŠ?Áíˆ0]m?Ýgeætúº?³)—ÎÁ?´e¨º˜1? ¦JEã'ò?Ý/ê˜(š?²¡¬Zuô!?ÑYXDÿRJ?¯1ɺ_û?ªzõ}eÉm?¡½¦ßÀT?嫤…Ó5"?²,ÂƒeMIXED4FGL J1840.4-1139¿èà½F¿NÀlÀóz¶À:™[†8"À;ø÷§kê4@ËK;½›W@'Wɱh?͝Çüƒs½?ëkö}ö%@œ(²¦°Ù?þ8›7(‹:¿ïým´8Q?ïÿñ¢o+1?ÝKáÕÈt¿çW½@½µX¿í¬¾¿ÃÏοïµ{A¿½ñUNASNone?ž8aËk?•ÆBÏEhŽ?ÙÀpсðä?ÆÊ-²?â/Ô/V?Æá6žo?¨a¯¤F;'?­¸ÊlVq?Ýç+Äe0m?ÇÙ	ÚQù%?ßžFÛb?ÅÐôéeM¦?Åäë
½|?©²—¬?ß!@Í$¶n?´†3Ppx?ÕìI«UêÔ?²€'ö?·Ã¡]"éç?˜o°þ;å?æLݺlM?²#N*-Æ¥?Êê¸g‡p?®‰î&T?Žõ¸#S‰?…(ÈDS¡P?ß	úÓxì?Ʌ`ÐWúF?àú¿,ñ?ÉaY §¢?–Sy~åò? ÕNϼƒ?Û¦ýžÆ?ÌÓ`om(?á{¶€ôËÞ?Ì"¯b-ǎ?¸—Y7'­5?¡]qnYd?âSÓÙT^?¸¸H¡[w?Õ2ƒ'Mo?¶×qÿ<Z?›\GÏXŠ‰?‰-»·žÈ?èaá~,"?·-LôX'?Ëkd?µ‡Ghÿ…ÍMIXED4FGL J1841.6+7113?ɺ®š»5@:Z–=Ć­À;tµcú{\À<ö«Yµ}ü@ ךÊF4Ã?ÿ׉¤Y=?Â$$wƒš)¿©CH ¢"F?ççf¬ƒ¨?ÿ¸Bi\ ¿ïìÎ?=­‹?ïüZžÜúl¿ç÷>Ælª¿ÊkÒ6?è¿à@H»ÊF¿æ&ÙRíÞUNASNone?ïÞ@Ãû©?ž¤€|ó?XÜÈ}ê´è?ž—v¬?eP×·£!-?f;<H[?ïÓ°ú?s» Ì"?JPA•Ý[•?Sþë"P7Í?s*ŸaçV?p¾ŽmÛï?ïonóãE?€a|øq;è?`GxL0qð?YÖÒºð|å?	PVq¶-?Œ(y'.i?ï'Áƒ˜{a?kN3#¡Ð_?p…%©¿Ïâ?UŽ,×-?ƒMN '¤?i®[œÚ¨ð?ïÕ4Y›I??‰Šgra
º?Xl‰ý'"Ë?‰
̃3£?n•a"s?d½®N!î?ï|èíÙ{¡?Œ*Üꪗé?]ƒ›Åá©?ir¾ì=ñ?"ˆ3 ?‰›ô"qO?ï+`èy?‰çÕtJ±?fD&‹à†?^­¸…]œ?œ2Ë ¼?‰%ekôÙ?îµÌޝÇ?ˆ»HÉ"?ˆh~<Ȓ"?v'^H" ?%P/ß?…ògžSAGN4FGL J1842.1+2737?ì[‹cmZ@,+ææS†À:K½R†À<ˆd•y@Èü¶õJ?ü…Ö|?Ķ"‹ë[-?ä†ü^	öy@eê«%)@ÔCíë€l?æÀv蔩p¿¾z% x…ù¿©½XÚ©¿â§ÿ¸ÝW¿î͐ ôí'¿ïžÏÎß̄UNASNone3FGL J1842.2+2742?̋A"Abm?ÃÁàúEÔ?çE8§Íu%?ž̬ʝ?©o2ÿ?«Xkh85—?ħ‡mòø?Àˆ­
>××?æЗle%?Ę¥™¾=Ï?À«Úàxs?¶ÙfýfÒÛ?Ó
†®QÙß?³"w'øY‡?ãóŽ¿9Õþ?´6°iøhÈ?´9oL{õ? ¾®šëOÛ?á4"؃J‰?ªèˆ5¶H¼?ÖyïÝ?ƒ?ªDmn'?¼w)Ë3"J?•T¨ƒA?ÁŸ‹…¥q?¼ø)`»E€?éäÆ_î?Â{Kù†Fß?«9Á#ka?ªX3…®ú+?´Éߦéð;?¸— Ë0"?é-šñ™œ?ÄJߓ45ù?Àä¤d£Ã"?¼]pÀÔ¾?ÈÂ&D| ?°*SlŒæÆ?ç°é"{Ð?±îÓ`¼b¯?²u2þ	NÁ?Ÿ¢Œ°¯7?ҖßÌ?'?®zV}"¯?à¸pâkD?³Ì†%Ó·?Çð|ÝÔº‹?¥$‡AÿßMIXED4FGL J1842.2-0328¿ëïäŒå‰»?Ý:
b>8 À8hÞ4Ô#À9¨XŠÑ @Å÷ùñÉ@Òa¤_Æ9?õ¥ouÙ ñ?Émµ$ºt†@5%1?ûrEî¿ìxÄ'6N?íÿ*¿åc'K¯¿ì'<ðKW¿ä • ãû=¿ïÿÿÊPËUNASNone?Ák^yCI?ÊÑ[Üʜ?"»jŒ¬Dn?«SóR_­Á?êÿM
WŠ?˳¬6̒7?°"'Y¹™d?·¹'¼Pjá?²Ú¢‰"xT?¶cî}' ?ë fÿ™?¿Y›|Ȩ{?»\ȋ}*?¦Ü­å'?ÈìTMEiR?±üN^vœ®?æcS6?²Ê€‹‰ƒ?Ÿèqðk?Œ‹o/í?‰‡ T»?%ŸR¿`@?kԛ?–šœxò??ºPUzRN?Í
³•ÕP?–eü"vÛ?¨mTy t·?ìšÅ5 @?Ím¹ò÷Ñ?ª…Ê¿2X¸?³€³ÆJå?¿©ôRIÊ?¹ù/8ª?êbdÉ®4[?ÃÙÚM$1I?·£É;
kO?¢ãõœ"´?̓Žû4?µÍy׺˜?媣UÕY?¶r5´dB—?GÎSh:…?ð¢ãxû?"p¯-h7´?œüz¯Ö?ï+þÐÍYÝ? sM<OTHER4FGL J1843.3-1242¿Ñ¢çöô¿ÀÿdIU´gÀ9Ñ{m^¨,À;pSÒ+í@Ž•¯4@£þwiÄ?Ì¨¯â?ÒåAbËÒ@'ö¿ž(@#V/ŒŠ'?ï;Eñ{ؾ?î/¥>éIÛ¿á<DSìç¿å«LŸjéٿ퐩e¿wz¿âÜþ=ˆ ËUNASNone?ß#=ØäÄ?ÅMÅä-ð?¡Iþ@2A?"»ÍËb?Þ¾œú2qÓ?År¿ x?ß(ÿÂ\JH?Ê5V—?¤‹)¶?Æ8¿‡‰?ÞS½ì#"?Âàç'¨!?ã·Þ†¼$ç?²Ì‰
óB?³¦FM²´t? SŠÛT"Å?Ó¦±_ˆü"?±u`c[Þ½?ãÚÚè!´?¤†KÇ?·0"´‰Q?"‡SêŽ?Ò~Bʙ°…?¢O*e¨R#?Ð]›ÖN›?½×Üö:¯S?µeXÚ*¼?ª7ˆ|‡è?åP&/¶@?Á	r…³º?τW®ž?Á½pKË
8?¬ƒ¡¸(?®‡˜´Ct?æV¦ßõ•æ?Ã8hãT‰Ö?ر!Ü°?µ»?cÖ?¹¬4Çu?¢"lwÛ*t?àÝÜ Ÿ)H?¶		ӎ>?ֈtàŸ	?«ç`ÂÆ?Ä8Y–Qï?¦¦¼ÚÌ?ßmnò•Í÷?®¦S_zCPMIXED4FGL J1843.7-0326¿èÕʱ¶?¹hšY³À8/r&À9|_æ¤í@W­»åt@ºd<Àz¯?欂ªiËv?¾²pK˜?ûV'QúŸ?ð•˜/âè¿mÜ	‰IGû¿Í—Ðk½¾<¿äÉh^Ž*Ñ¿éªÃø贊¿íþVèD!˜?ÜõÇb)ÀÄUNASNone3FGL J1843.7-0322?~s®"8e?¡KãÝy\&?k7¶À
ÿ?y`9ûs.C?ï§â+ј?¡ÊhoZIÛ?¬ö4mÂg?´Ô³YGê±?ªØeXàœ?«†Ÿ@ømº?샇F–ù?¹
e`óXÿ?¶í€/Œq?£€ Ò¬Œp?ÅVpÚ³•C?¯á'"BÍ?ç̳µ­)!?²ãüÊfL?…&‹!_4ê?sX§zÕ½?ˆ"ÁÃPċ?'uÈ=JÖ?ïJÚÌ6FZ?ˆ^óÅ"ù?'æW#.¯?¦ß4IüŠ?l1)r/y?{‹#õ™p?=<Bô?§W7!éچ?ž<ÇÐqn™?¥l÷8Öí)?­ŠguЩ¶?²'pòÄy?í5sJ-(`?´Ðľx?²?9™Ý>è?—
雼>?Är´›†6n?±%éÛ@ý?è›k¥âʇ?²9q}Èb?k¸®{À;?aÔ$¥^?|¥^‹‰,?†]îøºŸ?ïªü"ª`U?†Þ›œÍ,xOTHER4FGL J1844.7-2110?édg
{.À +éȆ/À:Wꢠ©À;³§¬_o@W欜֐@Ov¼Ï)?ÊY&âÂØW?ÌÒ÷_Ÿù?ÿ'zH›zD@0‹1vðw¿×7¡2À?ïû@>Æå¿ç¦âøˆ<z¿â¯Dü‰Rú¿êàx`cíæ¿ï÷#b…±/UNASNone?çXò՗?Á|£Åþ ?ž;2W¬it?²ãÿ'áˆ_?Ïç9›¾H6?À	#Èiw?ë¯h•bÐ?ºpc;ö!?xc7­«F?€;ž©]?ÀA¡D?¹€^/"SÂ?ê;~äÀ?ª–åLYý?ŸëŽÝ–?F߶-?ÃÖLÞßÁ?§¦±öL¦?ìù¥ýnïç?‹Vzóס¿?—,}'š)‰?sùï_ëÃH?²g°²G·æ?‡MºqK3ê?ÞUÕ$	I«?Ãz:}n/?±Ã'ü8#?ºS…tYÕE?Ý9a®?Ä¿zB«?æ'øÔQ™?ÇñG&@l¾?'í^©ê"? XœÁeg?ѽ8mTÅ?ÇU¾9¿?âƒ×ª:?†?´
/Ì?²Ö‰Œv¿|?žÄš¤0¡^?ÖB®HÛĕ?³4ÎO!?é[ï¶Ërs?¡ÌDº	ʱ?©ßúî?'ço ?ÄJIb¨u?Ÿ+^1÷dtAGN4FGL J1844.8-0957¿ÏIµ%TVÀ‡«¨À9€_7ûÿÀ;Íì‡}7@Á¡w‰yf@Ö$o…Ê?ÌY{ÜÅ=a?Ôn›¿
Çi@tòñ#Ä*@¦Ý>ßå?ïæÍ)Á¿ÞôC~"ë7¿ácÍ.ò\¿éÐÚB×%¿ã#¡?€H¿ïü¯ž=Ã/UNASNone?ÖW)©Ç?ÃÛÈ{ŒñÉ?|ïÁxç?'£t¾ú?ä^†¬	¼J?ÃÐhöík?ß"oš'ð?ì/¯H¦?™ŸŽ4½u7?–JøÀ©O…?ßHs¬u}?Ã;+Ð}?ÜÔVÁ$Dz?³¨"Û%èã?³Û@+$'? 'ù)ˆJÎ?Þ4ÅîÐòe?³>-¦ñ?ØE˜R>2¸?¤&ÿà $?«ˆJHÅãò?"q(rÎ?â$¯2Ð5?¤eù©Û£X?ÉÓ]G¹?·C	¼×À?"£~Ö¼é?‡Ý:å "?èî2Îi?¸&æÆ3…²?Èø)¯Hz?¾'á¨H€o?¤—cö?¥eq"€?èóäØv?¿i\\n¸<?Ì×?ÐMh?­qèâÉK?µÙÜ­N?ŸrÈPd'?ætäêŒ?°´[e!/	?ä]'g"ú?žÉø$"é?±œv%µ?"b*e°é)?èöu3?¢Y¬ªÔ¢OTHER4FGL J1845.0+0159¿êÝТ'²<@¡®ÁIÀ:Œ°càz)À<:.›ô½­@žªÂ`ã?÷}}8Ð+?ÑüU›½á"?ïÿ?`h¤@¤Æ†"Ä?ûïm£Çoì?é|Ÿ5åÀ¿ïø''ì×.?ïÙ8`C·¿Üê_d"(¿ïþß~«+½?ï 'àðUNASNone?ֈT²ß»½?È	ñ_B¢?ȳ""?Á­Å~,‰T?ÝkÑÍñ¸?È:%ò>‡?Ò"‡¢?Ѕü4T¬'?ΓŒ(Ö?ËTœfÜ?ޓí4m½??Í@Ý¢ö¡?ÝK‡ª{5£?²ïç…ÀÛ?ÐF¶j,;?°-id®?Ò¢1Ÿž"?¯Ó;pO?ÛEÍ73{‹?¶*4~x0?Á"]<û‰?°Q'쯪Î?ÛðF®°?»%™N'š?Ç=?ça?ÁƕaaÕï?ÈÁiÑCþ?ˆN^$?ä`»µ*ø?ȍÃ(ŠÒ?ÂdU»¯E?Ç~Ûaåù?Í=ËÊe¶¶?ͤRxP|M?äwžz²?ÏwÌ¿`Ó?Ö_ñ«1%?².ª|Ï?҉öFvd"?³ê'ÃŒh?׃jG?³'—Y™–?Ëfv
š¿¬?µ3¹œT›?ÄĽ¡X!L?½éJxáò?ãõ3CGÂ?Ãný(»OMIXED4FGL J1845.8-2521¿ïܲMùÔÀ$=:uFÔÀ9"Bþ'Q~À;Ì"ð½m@Sj¯÷)@DàÑ?º×ý­j[é?҂A©¨…@Í%îÇÉ?ô@gÌm‰?ïðcu^P¿àšdÃÎ÷¿ßn{=Ž¿â"º?+Žú¿ïšˆ!L*ü¿ï›¡æoUNASNone3FGL J1845.5-2524?Džcȍ‰&?¿ì³˜¯u	?×Ê£Øe?ÈY"¢ŸÛ?ÜrÎx7c?É\¢ÍõÁ¹?¶F{O6o?·^ls¦?àTæŸ?njÏò:ï?ÚhB')kg?ÆQB¡ÔëC?ÒÇÿCÓ¥•?±e­Âÿ5?Ú&À] D?²Õ>."¢ù?Ó@`(šå?°±!¬•?É÷BæžHð?jßÌø¤i?ÚÅ­Co–f?«­Š|Æ$<?Ø>±IAE"?©¢¦þD´?·™ý¨œH?°ÈÂĦ±²?݅ÑJh?ÈÜìR	s?ܔ£/ð]¡?ÇýpÈXã‹?¨ÂýÝÞ9?±ëA×æ±O?á	ëL)Ï?ÎMÄâ{=l?ÚÓép5`ú?ÍqŠHc­?Âû‰ô5?ª;`ç?á©×4¸L?¶Óïx­Âš?Ó.ÃѕMH?²U½)Wµ?²ï'gä?'°‹…R?ßvH:p-(?µŒÄ­-E?ÛÍð%
øÞ?´¯­6—\LMIXED4FGL J1846.0+0507?åÿ!5"Ç%@HüBÜ£À:8ÓMŽÀ<Æ
:ìe@fþ¥7§?ûIR>'5G?Ì5?ÒÓÍ?ã'-Ê=¦T@°—"ìck@`{—%  ?îž›aö¿ì´=õ.æ?Ã:öËù¾¿ÖÿÊ{
èK¿î'Ó¹PF¿âúy]¹ïzUNASNone?ààTŒ|Ù"?ÄuWð×Ä?¸ÙPás?¬%¡gRÑ\?Ø	®Â0ù?Ä1
@QÌ?Úuçí9ª?ËôÔ}Æ)?ÃúËQ'[÷?Á]bøƒð÷?ۍ}oJ[?Å_X0CP?äP×␿'?±­uùQF6?Ãÿ%†›?§æ‡Þ1ñ?˦¡P-{?«ƒÄ¢à(ð?å—wF?£Õ²:ڄa?¹Çvþˆ?šÿh;¹Ð­?Ì¿ÿƒ£¹?¡¨î{'´?Ïür8Îõé?½ÊN¾æ"?Ƹ̆©?¹ yƒ_ג?âR°mð|?ÄVƒ—L?ÌeÍ@]Ç?Èôý(Æ?ÇaH¯Ç-|?Æ<A¦àÌU?ã:þ/?ɔX°"û‹?Ýÿ["nœ?³q¯Î¦á?Êiê2Y?°êòÖæoû?Ô˯Ćà¸?±‹*t€'?Üf%"ú+?¯"Í't°L?Ä;+Üõr?®¼®ÈZX?Ù×ìbƒ?±¬jx¤ŒMIXED4FGL J1846.9-0247c?µ 7ÿ†ï"¿Ñ÷u¢™r'À8Ž€µÀ9þ±¨ó@ Ë´Hòb@? äçuÅ?ÊӚFgÃ^?Ú1à!é3á@LfÓs¯û@
5^†ž¿ã€¿ð©K?í§\€3—¿âp*ՖŸê¿égDýàëé¿ïþ Eð¥?ïiQ;UNASNone2FGL J1847.2-02368?»š«á½?¼_E0œç?£ol¼š9?£ùÝßï?ën5ÇPûµ?¿;(Žj?¿|Çôa?º³³þª?Ä.E9èPƒ?¸½—fÍp?ç߇hó?Àȕ-þ–?²ÂN]tê?®ç	.¿ë?¾TÆÎ'?¬-±×›?棺:µâ?³¿wã"?¬ë×9¥?"
ãñ¼ƒ?¶bÉ_J?˜eJ€®p~?ënv5ƒ?¢U˜bâÎA?žß3û±Æõ?ªd-?íð?£èwæ%`?£IX#,ªÙ?íÊ~á²b?±UÒ¼ZKÁ?§'
»^5?©IW
¸?ÌZ"Isf?ÄÿKÜï§?çq:R6X­?Å˒>ô ?µH+¨½]u?¡-/c?Á­¼;Z?«b†¨"A?éç<:?°"?ºåuŽ?ŽQ%N¨‹x?{êµ
ÑNÄ?¹Ò ~)?¤'::Ñr?ìLg·Í¿?¦0hj²nOTHER4FGL J1847.0-0625¿ñ""(–D¿ÿ-O#SÂÀ:GwÀ*ýÛÀ;Õ+y*ŽI@k÷τâþ@eXê|àü?ÏÈ÷ê‡É?àþ_o×(@¨¯bk/@Æi/œY¿ïýêªr/?ï¿©~+V¿ÏåH U5¿Û¯Cdƒ¸1¿ïiÿºùf?·Qx!$UNASNone?à‹§áœE?ąȒ'£½?¾^¿9LŽ	?À4"œb!?×Qé£ó?ÂnÆÿ{?ßÆÛ±—T?Ɛ7MÒ¤[?£PYb0œŒ? ¤¨+áW?ÝÏ"Îš?Åq–¡]³?ã0T]$s?²Ï2¥<±?Âç–eæ?¨½ÝÊ?Ð,p
%¤Í?­ÂÆ+Ñr¬?é*pm­D?ž˜£¿&4â?«‰=Ͻo?†MMœ³,ý?Äsø{¸nW?›O61þÄ?Õ^n\ÃÈ?ÁGÔ¤v[@?ÁvÒ^ ?¶¯åïr9?á	+Jº?Â]̗{dÙ?ÐZʋÔà?ÄdË!Ú?«#÷}Ô˜?®EpÔQÇ
?æ ²£3~æ?ÅÃUˆPO?Û°ó('V•?³Xó~l‹?ʃŸsH'?°PQ]2
®?×
=L´"?²É¯ENe?â<~E«/ï?«²Õ9^ħ?¹³Žf¤h™?ž˜`)M'?ÕÛ…ü?­c·Q¾ÎMIXED4FGL J1847.2-0141?ìŽÔá0:?Ē®Bóð}À7å·lé7À9|¡|¼ê@Œè¹èC¡@ #¦Î5ƒ?Á!¯}0­G?Ö92¼î¥@}¶åû@f·Œž´a?±öí ™¿½?¦´	\u¿á ÔV.	ÿ¿é&Ébµþ¿î"]à…ç5¿ï¥íš¢®UNASNone?¡ôU؜µ?‡©s]CÍ?Ýt¶¾Ìº?×)M¬0J?á`¸Fi?ÖÚíˆ?¦,ªº7¼?°E@RµÂ?Òí#ôÔ?ĊœÑ‡q¤?å&£d7{Ü?ŀŒoŽ?´duì'?¤¬X	¦¢?ÙùUnú{?·GBn"Ÿ?àèº³?¶¶ýAǑ?w:­M"?_ç09ÿa<?¼§Çš2ñš?›kT‹ZZ?ì<'²*Æ8?›ð§²?y\ÉN¦øÆ?urü瑳?Öw+-ˆ×Þ?Ð7bT*q?䑰Öeìˆ?Ð+ðˆ,£'?Ù%q6v?œý"צ?Öü2Ýð-?ÊB6=K1y?ãû/|*¯?Ê6Ώ*æð?¨*;É<œ?›{@&T¶?Ûi)©
"?»ÀW&5&†?àÈÉH˜‡?»b¦4Ôë?U¼P'´' ?ENˆwO?Ãap÷þ™?§ÿÅ­Õ­õ?ë1‰{z…é?¨øÝlOTHER4FGL J1847.2-0200c?çf¥v»?Z8ž'6§À8`§GØæÀ9³a°ôÿò@ †l(T@å eÑ1?Û'¾Anµ?ä'ô>UÑ@ŠÎ$»¡+@›¶‹lÛ ?í")à¤&¿ãւN8ó¿æ›»øi3¿è$nß±«ß¿êLÆ¢fFÜ¿Úöüᒁ¢UNASNone<?²zëÜòÊ?³¶6wG°?—D˜¯e"?£³BC?ìö}¾ØÔ~?¹f@€?¢Í?¬É6€ŸÁŠ?µ"œ] ö?³c'?ì'œnE?¸œã«)?–ôß̕?«n?…ž\n?Ä/4q²Ûñ?­0 '?æSÍ&[UÞ?²ö@Ԓ†-?ŠB!k=C`?pxeŽŽ÷?®i:û*b'?˜q9íÑC?í°cÊw)z?™–
a×$X?¡ʯ î?ªÃHOá%?"åàçŸÒ? õL±c¯?îOtTe²â?²ŽJ¾¼ª?"'«¶,?&ö'W«Å?¾£öƒ™@ó?½·¿CTò?ë†ëї.R?¾ðy`zO?¹ö*‡E·£?£¦X"Ë?Ç:6+Ný?±G"ïœæ?æò­$Ìú*?³'lt/?f4´P Êš?U¡GßLâ?°=™"?¤æ^^?íéc©Ñ'Ù?¤ìúÓf)OTHER4FGL J1847.7-0125?ï}¤#=ûA?ła€"¥À9PþöÅÀ:z¶ƒn@!ê
¬»à@@Ca~ ?Ï<â()?¸.žp?ïÍ4›èÿ2?û;Tiä ?¯òlÄyl(¿Ú|#¼ó'¿âð|iÝê,¿êSb}¤¿àµfÿ"s¿ß½×üÖªÇUNASNone?Œfy&t˜_?†ž
±>\ú?JÝÏ\Ö¼?PU`,zO|?§•';?‡5J*™Ò?°Ïxš7Ҕ?º!'Â盰?›BH‹a?£PœÎÍðô?íþ¨‰mõ?¼¦ã6Ï(?Àq+úWõ?§Ä,´ Õú?«fùlê™N?Ç·òǞ•?ê-EjdÅ?«ÍSWö?£Ìÿùò?ˆûµNë"?€øxǛñ?l|¥NáT?î'ô,äq?‹Ú·="Þ?‹f–ð™q?†ËßÄ(?[d¶Î᷄?ŸìÔ'¸×?HõÅÈ? Í‰u?¤™}N?¬HYlû"m?œ>«‡8á!?«ìµ+¥Ú?íÔz'\'b?³àÅμø*?¶šM"Ü–C? zRÔ?§°!÷DÇ:?šâ•5N(?ë±´.+¤?¦" - `Ù?†Êº[­'"?v;ËÕ nc?|Ù1cjØ?t†Q©óo?ïk"õð©î?€ºxDàßOTHER4FGL J1847.7+3543¿èEéUˆ#@0!†¹ÃÍÀ;Ÿ¼
éÿÀ<Ͻ¥œà@!j\‹ò?ñ•:uFÔ?ÞÆÀQ>a?ì¯:€.Ž‰@P¾yLòø@Ú%ñ]É?ésÌ`@\'¿ð?í—ß…65?ïÿû˜'2¿ÞÀÝ`í²¿ïþâ~dßÔUNASNone?ïvP
Ѹ?©æ‰-Þ?e¹­«¥?tƒ®Ü5ó?šÞÃó¡?¨áԃÀãa?î'†;\¼?®v³'l˜g?…¯¨'¾Š¾?•ò~ӓ½?¡sÍznFŠ?¨KêÇdy?í"­à+,?¤2%ìù'þ?z1Ó,ÒaÝ?|ÃÇq~‹?µGsÊ®2?£ÂÈq[R…?íaœBžé˜?£'g@3ªZ?x¸gyûà?r%dcºä?³gä
"?£A"ÎBh'?=Œ¨o?«jæ¸7=?|XËbŒ6?'­bRËHý?£|ɪ-‡?ª/q¦™-ú?ìæ ÜՔ®?¿?§ŠÈñK?™ñð€'²§?¯k/ˆ_³º?²R|ûXof?·«éÃ^¬6?ì3‹9Hdâ?§¾vØ*w?€RO•Uók?² D2OÚ?¼Y\A
UB?¦´·''ß?êWA]ˆ2?ºóè<k?¼"G¸?–¼šÏ©?ÄҞÈØvy?ºŠÇA¸ÿAGN4FGL J1847.7-3433?ÜyDW¦b³À,˜â~ù˜À;<Ž%ÈÀ<£yv
£W@‰nMægÓ@.Qúž—/?Ïê¯ iú?àh…à19@MZ%æC–@L¡°ƒ•?ïûñ}†=œ?ß8KgÝ_¿ÑúÍ%¸ m¿ã˜àkæ(¿ïìÇÿ]˜·¿ïÿàöO}UNASNone?êFù•W?ÅðÅ­ý1?·¨}öƈu?µíj­ò?¶µa}Õ?ÁJg&f?é&#!1è?œê·î;?Àí"$‡U?¼ƒåà˜Ì?´ó¾¯ ì?³Li Ñ÷?è°c G†?°cv	+)?¿@ò*»|?¦¾º†_P?»<͝(V?£¿DEá?çÇG8	?¡/<ó?A"?Åëƒ0Ì{™?ž™±vÂðy?»8d-H…?"­%<¥x?ç¦é¿²ï?¾ZÜ3`ïH?Æž(ZÎ>?¹Lç{"Ã?¶u¯ûü?¬ÅƒÉ¡ê¹?ãBÜ¡´£¿?ÈçڕôYÀ?Сs»—"ú?Æ«ºŸ^æ¦?Á±¦ÿ+?¼J#åbÿ?äv–"f
?·wʵòõé?És•êɞ*?²ôlX·V?IJǞ9¼?­Ë¿ù®?ßébîüf\?­ÈÉDós+?Ò)k)ªÚp?°֚Ÿá¯?ËÚcÐ×?å?¦@·Ï;qXAGN4FGL J1848.2-0016?ã‹IJTj™?â™X {öÀ9@©-À:…! 8B@l¦Ð
ôà@Ó!_Ìr?ÉA¥Ãt?ÑâÊe€@XQeMa³?ñ´FÁZ}пïùÚí!+?ïðBRŠçO¿äg¿Sg†¿å`5•
Bß¿î/¢ŸÒ˜¿¿ïÿÍui8©UNASNone?·×W‡~΍?±Eœª£µ°?ÁÌÛ̀1û?¼ä»Éøºš?è'ÞԜÐ?Á9þô'8§?ª"v`'ÂU?®ÜÌÐüÒç?Ëü
ýßê?½$"aŠù2?ç'9—a—0?¿!ýÉÍq–?ÃôGv\S?¨ýÞÓåŽÈ?Êfö6Ü?¯qÍÊ9#×?ä'ԁT±ç?²+7Þøû'?¨Üç	)˜?ˆvO2zù?ÈtãþRçë?¤Ô'Ðî¾?èTøô)]?§œA ¦ž?°¾~,Ú«?¥ùÖ"Ð?Â×=ò‡z?»ásøË-e?égzlÐ\?À_œ®Þ?—nc	Ê?¸~ý…((?Ðdò)õê?ű€|Mi¦?çãz@ìb?ÅÇm`ðI˜?·–wMh?ŸFU':1?Êàs•{?±h¼!Æß?æ‡EŽ$?²~D÷¨Xÿ?'ÿìžt*ç?zæÅ%"?ËT躔?¯Ð—qó¤?è®+`ù6…?°†º¹ÑOTHER4FGL J1848.7-6307?ìފíâÐÀ7³c€ßÀ;Ã2ú(OªÀ<ààðp@@!›?p-d'?ýÎÇä/¿á?ÐÖ€Ú?ªó/bN?מ§Šóäi?ùÅ¡²:$?ïÿùµc#¼¿ïÿùµc#¼?ïÿN>úg¿Ôú­ÛšðÝ¿æÏW´ü¿ÚTË^b¶ÙUNASNone?î­u'?µØ֚{ÍÉ?2ÍÂlèm?Fز¹!
?¥qFÏJ?µº26Ž%€?ïVÒt¬z?‰°]¤w£c?bq'öl@	?jð9·§cÁ?‡N\úÁx?†31^0ˆ?ìï£}r?¥ÚJ&ÔP?_À§¾Ÿ"?i‡sf¨û<?¸á|gd?¥Ê6´÷Í?îlúåcÇ?‹S\vã+?p]"êe1†?aàŒ8Ý=?§$«ÁEw\?ŠiqfRM?íðÿ©~¿?´ÁÛ!yLr?<
…:´™¯?<§€/Ó½?°[ù›¤ñ?´¶'*–N?îäüð0Ì? õµ—éü?pڄ‹Œ…ö?€·–0Ï?Ÿ)ÝޒÓõ?ž•`3xP¿?쩟—ú!?¥ öíùy?`lΌvåŸ?gZ¢O«?º/œÌe/?¥™ÏãAS>?ëÇèÔë?§\ayÉmè?€.C°þ?}~ÐÀY?¿ÁNá±Ø¢?§"Tg3¶AGN4FGL J1849.0-1826¿ìâÝK[YSÀ-s!_ÌÀ:hÒlHþwÀ;ä"îA'›@ÇZeý
@Ïw¡øì?Ïz!™­»?ÖÔx<ҙ@@¸â4=@In+ߤ?èÃêXÎÎ?ïû³4uR'¿à¶e)O…¿è@Åø50¿ê3^1
¿¿ïÿ¶>@£UNASNone?ááÔÔWŸ?ÁŠ²mrk¥?¡èöÙMª&?"h4!
Ïs?Ùÿ9d•<?Á%…ºž?äyN[ØC?ÃÞk ÃÉ?™í»lÄ?˜NrÆSÞ?Õ{°àˆŽ?Ã.^[Ä» ?èõûÙèÙ?¬FLfFA>?«œ;4‰tˆ?˜gYØì?ÅA'uÿz?¨*/"tŠ?éO§Ï3Ò?€ÿ«t?© ÐÓ>A?ˆÊ\ܯ*ì?Ä_Å,ÅZé?™¯io æ?Н·`~ðÌ?¼[€]¢6e?´?×H‹;?ª£`厥?å-|Tå4£?¿¯{ÔÈÕØ?Û'vH~|?ɯø'ÕE?§73p/÷?¬UÁ	µ?àøÑ«Œhâ?Éê"-üN?áÀ…ÄÙ?´–9
5õ:?»0iÈN@ˆ?£«ôª«G"?Õ²Ú:CÀ?²®JŽ'¬?âØ/¶žY"?¬¶ÐÍg›R?µ…!bÊQR?œœŽ¾	À'?ÔîX9õ;£?«"yûá¼MIXED4FGL J1849.4-0117?﹗S¡ÆA¿Â¨†z'À8T‰.‹CÀ9ž¡´N`@¿Eß]H0@'–é»ñ?ä@¯¸k?·ùf³¾3?ùg£áñø@û÷­K'F?ì"\
G`¿ážä'åp2¿è°‡A}Mß¿æ†o»y¾2¿æċë[-M¿íëÏÇSHUNASNone3FGL J1849.5-0124c?'!@áTjÒ?¡þÛsËØ?R¢$J<°$?XÙL™U
ý?ïm¤æ©Â²?¢%«"Tm?¿ÂȽHÿ?¿j'ùS?œx>Œ? þÚ±©ë'?ë#å>#7?¿¦`*Ñԍ?¿F¢Õò)B?¨¥œ ùÎý?¶‹'gGÂ?¥.ælaü??éE¹xKô?¯sâbÒ?±\·¾D¨?˜uUý?záØé~?q…ºÏÒ?힦öƽ¶?š–PÚ{¯?–"YcžŠð?°
Š¸LÄ?Tø¼¯"??`,À
›1C?ï@èÖ¡?‰?°!;Ž‰`µ?´,?ǪÉÏ?²·›Ä3z? ô%¨Çd!?«"‰ùW!?ìk5¬pr?¶›(õH•;?·'iÙQYS?¢ =§ÊAª?µ•Ëaú?¤çÆ\ÍÒ?ê[d2¸?«ÕWÆ}?š‹²ÒÚëº?ŠÑ›¯ôO?q2koŠ0?v±h/"?ï	='¡q™?…3æIfOTHER4FGL J1849.8-0952?×¾là†›™ÀŽÏÃøÀ:fc$'†€À;ʺà;>š@ƒ‹û¡K•@|{*BÊ?؇Ï!Éf?ï."²‡§@
†Ã%"?ùœbCÁö°?îxËrK!¿Ç<™"ü.d¿æэ'Mš¾¿ï?ërªAˆ?àc¯ga8)¿å­j0öBUNASNone?âœ8·EjÝ?Æ÷Ò}™f?Ÿw±Ä1Š?–¹"_dƒQ?ØÐu ?ÆÔ~g90?àª'‰ø'?Éém0Ÿ?¡¥Z…0Â?¤—CÁs€?ÜwO?ÇìnȊ?㯄c7Ãø?²	æœó?¹i؞­£¾?¢¨ëÑÝø?ÒFS ?°OñÆ{j?âÚ\™+?¸þ¨aŒ?¸à×
?±9Ÿgoî?ÔJϊIøû?´×'Âå·7?×r>PȚc?ÇE¤jêí?©Žþ'sÛ?¥)N$ry?â­çnÓa?ÇÿCP•L?É}5ž?Åp.Ȕ?µµ:s&9ç?»e›Îs?æéød*L?Æ€:'»?Û÷ïunA&?±»°‰!Ç?Ã9øV4âW?©ûZ33P?Úk`Š.m?²Ï¹pN?É×VÀ£k!?¸R*ãœÏ?ʑs`Ûô?ÄÒk¶÷^?âåÍx)˜'?Ã(	ÖºÚMIXED4FGL J1850.2-0201?í@²3¿åg|`£®ÆÀ8ïcF÷5VÀ:#Mçê_…@ ´nÒñ	@ñhr° Å?ÆÎ8‡°ãã?‹«íë;³ñ?Ðô:$/³?þÈÍK¢Àµ?ÚºÔè$A(?ևÊ#ÐÔ¿éJÙ!ï¾ê¿éì°Ý­ð"¿ÝõÝ%O›¿áÛÇqC9;UNASNone?9OßC?€Ÿøٔ? $á'Îö¨?».˜™¿YG?î€ÌªNXå?»=áÑ°{!?Á9f—Ó`?ÀðŽ›ÂFj?"i	›'?™ö	?¡?ëèæD(_?Àóüm	©Þ?ºýÆ\ù³¾?¥]¿Z†O?¯	'b? 'Ôވ?꯵âqò?ªþ&"œã.?Â)‹Ÿe?£#zÌàÀ?‰YÑ=?q	ñM¼»?ë8óD8r?£ªP&,;R?ý©8ž2?š÷cmEzI?fiL"¯Â?rÅ&ç‡!?ïa©iàV?œŒÔèŽÅ?´UMÙ4Œ?³]ˆ´S‹?'æ±™Mk?¢ófÅþ?ìç_Ézn?µáÔ¸"á˜?²Î!W/ë?[ν$Ԛ?©ûgâ3ß?šjAgSvJ?ìL€b€?¤{Ù:$†K?ª˜Ù]wt?–#{C~?‹©œI‹ßÿ?|º3—Šâ?íçËù	¹	?˜vŽ!¢Y_OTHER4FGL J1850.7-3126¿ØÀ©ëmÄ À+@y€õ]æÀ:—žã…uöÀ<:g;x|@ùª&ڊP@ýã$ýæJ?Ò¡]•Ç?äÙ=ôWU@y…'Î?ú‹šZ‰¹R?ïêR^œ˜}¿·*1¬ËOŸ¿æˆ­'f¿çZ.I¿f³¿ïÿñ¢o+1?ê©}'QýUNASNone?éÿ3ë{?ºŠ»kŒ§)?À}ï*Uû?µw)V`jì?¯ôUQMi?©º'Åajö?æÃzÖ,ib?Íâ¶÷	?ÈÇwMijR?ÇÆNg…äö?¸U:·§oÈ?¼Žµ\e(?â4•ª»nÅ?²
Žì&
T?ÈúÚŒ'?«×9×?Ï®{¸Y?¯ÑR7mE!?Ù«GMéº;?¬Š'U~ch?ÚRÈ#ð ?­­]þ?Èáqæ?¤y›Ã¬Y?ã¼Ëì@'?Ãpê"ž?Ì
lÿL?À¿XÌ[?ÄÿÐ`¼>›?»&Sw‡‡/?Ú%£Qºn?ÑO!¾õ&f?ÜG*³ª3g?џA<	P?Ã'‡OâbÙ?ÂÄL?ÛJ?5ÂQ?´#ò¤mu?Ðë´Óu¢2?³•Ô ÕÂÓ?Ôîg|;?´QԗH;?¼1÷ßJ'ì?Ÿm	ò?ãp@[~š©?·qdkµ<?ÒP_ó?´¬ô®@"MIXED4FGL J1850.8-1105¿áÜÝIwîÀ•?9ѲæÀ:yx˜˜ÚÀ<"u]@–ú©T@0#Á¦(?Ѹ:#gc<?éj܂Luú@þ"'Ùc´?üý"åø?ïüB"ßοéwKáâ8¿É*QwÁØ}¿èÑþåxÀ¿ì»4SÄ£3¿ïЋ¾dª$UNASNone?¹ãöÈ2?´È˜™@7»?Ήtn£?Â$›Rg'?å!$"7ù?Äm³A¶Y?Ɍ8ï?Ã&9eûT?È%¿¨Þ\?ÁP¶ç2Sº?㓁Ú¶?Á0X¯»çD?×F[)òB?±"›ñÁ+Œ?Ò.å"xa?°®Óíœ^?֊›"³•]?±7t)îG
?ÍSÏÉ4–?¡r1n²†?Ü4…–Šù÷?«?¨Q6a8?Õ!'"Úù>?§³FO?¥áNÙ¿¿í? ŒXKÅK?Ë´Óڐ¸R?ÁÌ×&Ëyn?ç´¶–š?²A}›-»?²&؁ÂÖ?´so£š?Ì_å´™?Æï¥6RD?æ¦lþ?ÅC–ëòàe?͎‡¦Áº?¬Ô‹³×ý:?ÖÝ:4ѐM?¶°WK"?Ú[÷͒¬?µêJµPœ_?±G%¶ü_?"!ó´†ô•?༄þàxÚ?´@ߤWó
?ÚF¤9Z¿"?³6b,ûMIXED4FGL J1851.0-3003?é°ùærÀ*BÀð¸À:ö2÷¤À<;ê'Ù²@Ú<ü@:Ü$X¤Ý?ÁY«'zC=¿°<°	š?ò1r¹[@€
Y]¿?Ð=û"ˆý¿â#¸¿ëH¶‡D¿Õ][$éÄ¿ïÿü9¡â=?ïÿì»"UNASNone?ï †dÿ?–~§€#8?~MÒ©'0L?xÆ¡‡ -?"l:‰ë[?"š‡ÝîÛ?ïoô"bf¹?šãÒåÐä?c‡ˆl?nß»£É?!@²aa?™PT¿˜ü?í¡ëvŸÞF? Ì-s3\?ŠeÝ)'Hè?†ÌÊ»¸?¯GÑH.-j?žÕqƒr]?îýˆ—úÄ=?€üh/7$Ø?lBƒN{Ó~?VsœúÞ?œÆœ›§qç?£Ü.7Î?î ˜È£j?¦zúC¾ËÌ?'©àÌyŽä?¾¦JUY?¤¡ƒÏå?£Ç¥]«?î¨V[2Î?°ì³—ÓŽ?sºº<Ùa?"ômÁÂ
?£GJPâð?¯_Ì=a³š?ë^kÙu…F?«»…&Åç€?–µV:S ×?½É/т?¿_K¡á^!?©¦[H?ì®aÎë϶? À\Ǚ@µ?ˆ^pÆ.ð?yàu^ÆpÒ?·#mººô?Ÿ*6åOAGN4FGL J1851.5+0718¿È‹)iZâ@
i‰¡ÑÀ9"5´í³À:ÆÃhŸý@°¯þ4ù²@ýˆ ËQ£?Àdlü'œþ?É":·¶æ@½[û©Y*?ùPx–Ó?íU]T™à¿âÄÜ=ƒN¿èº«'OP¿á`‰½®vË¿ïü¤ávR¿ïÿùµc#¼UNASNone?͈ÎZÁlœ?¾6æµ´¶?ÅÜSú_¥?ºsâzÞî?ã&·jÌð?Áÿô6ÉÜ?Й£	"ä?«ãÑ©³÷?Îç9¿-l?ÀCøpr6‡?ßòÀi¤Œ?Á˖r¸•?×g2ÿ†³c?²'Fxÿ(?Æè|3_Ü?«CZûP?݊ØÂ_œ¯?²À…Ú«1?½"ý|±Æ%?™nŽ_ú?ij7$âì?¡Š—'5?ç ¿B Ž€?¨‹Úd$Í?ÅåÌ«[?·¬?̋ÿÓñj?¾ðf7 û?ã•ÃLàO?Ã/¯´ÒÊ?¶¼ÓšM<?´Þ¢3ÝWS?ÓåᎷ
?Æ:w Û?ã5uÚ]ô?Ŗ´{¶ôb?Ï÷ÔYÖX?®¾ÍL!â@?Çt/î–\_?«¼…¹µ:V?âBöCóR?²IGùg*I?¢ˆ$÷è ¿?‡1¥ZCy?'¤q˲?°@>øºñ–?è(T"E¶‡?±¥CW–àoOTHER4FGL J1851.9-1522?퟈—HmÀ6F(}‰À:zà,À;ä€Ø´5@Vœ.t\ž@ã7!Õ<Þ?Õ\ôb=ú?íþdŸfã@7Œ†‹ŸÜ?ýkûägs,?ïï˜p"¿Ñ7è‰ø<¿èj&Ìóc¿ërH½3«¿ïÿÚÁ,/´¿ä$ð_µUNASNone?ѧÄãÅ?Ä5Çø|¨ó?¿;µœ	?³?,´=&?ãD§Wzî¼?Æk^yCI?Ðq*´"u»?ÉÕ=S{?ѝït?Èv€Å=k?Ýðæ3È{Ò?Ædˆ.¦ö=?à‡M¢ÜJ?³º¸f:?Ä'L奦?¨›ä+;Ž?Õ¹0>Gtš?²¹º49…—?Æ°ž»8ó?¡X;æ?âø{ˆÕµ?°)ò?Î
aB÷1¶?§â¼CÚέ?Ǟ/a¬?¾§a†Ó?½üAea??´	KŽ-\?æXð´³{m?ÃnÏ d#–?ºuÀa¥ý?ÀQØ°êö?Ùm
šbÂB?ÏôŸœ	ƒ?ßõ…No4ý?̟íÍÃ?Ô^3ÑWÎ?²Nâ6µ?ÌGs3J҄?³ÄÅT—ä?Ý~•ñ?·ÚRc¨…–?¤7œÈyá*?ŒQE!Z3K?æ…÷*:Þp?µz§!RÇ3?Ðm²»?³Ø
,Nž'MIXED4FGL J1852.6+0203¿îʽLŸ?åcl2š‡À8
 yóÀ9îäùê<I@^ô­™Ö@¬À½ÊÑ?Àâ3{ØhŒ?ÃK¤n3å@o‹XŽ6?ó,c8¯ý?ã¥üH»Zµ?Ír!²lN¿æv÷"‹Æ¿è¸€å¿ê–ß~*R¿äîDنUNASNone3FGL J1852.8+0158?°"w0~œ?±ù?j?³Ôv'Ñ4£?´›'Ë‹?냀¬Iè?¼-ÄßB›0?œÍl¯ÖœÚ?¥ÅçÝÆÍ?ÄÈa<IÌ?·íšÙ§Õ?éç|K³C?¹¶Rbó?²RÙóè×?Ÿ±e¢£ì?ÄsÄVöJ¹?¯ÿˆKh‰+?蘳«œ.'?²~¾\û?'Lµâ»Ñœ?vÃYWwa?½l&Cá:?šYîÛUÖÀ?ëÀˆ
¼<?˜vT¬;?¡*}WÀ–?›Å"/À?¸. üÍ6"?µ±—Gõƒ?ëç"
çÂ?·ðÐÑØê?Ùv‡?•¥xÚc6§?ÄàoÃÿ–?¿dº0?êH¹QMƒ?¿|ö†ì?¯‹FP)?˜$U"Zîš?Æçø†W?´Ø:ð?èM	H(7Ø?µ¡1	)¢Ð?vw{/ìN?c[œ™S?Á¦Þ8Ë_?¤™AyÚÒî?ëiY‰Ds?¥$ºä0ÛYOTHER4FGL J1852.6-1159¿íÇÄQþûHÀ΢(´TÀ9çrüvބÀ;p££×e@h¿:­@Zñ£EêÆ?ÉSme^(ª?Åö/‡,.²?ý[ö Û­?øäC%ï}Ò?ïÜ5?ÒÓÍ¿´¨JŒk2Ô¿èûù`(´ª¿âwÆ´{G¿é¬lÚô­¼¿ïÿ¦<ådUNASNone?ה‰æYvû?ÅÃí{Õ¼?'jÆVíËÁ?‹]c¬yz}?ã¢dÙÉ_…?Æj©ºà?Þ»VXãW9?Âf+ôá¥?žW¹XÅ?˜µBY¦@o?ß_.%á*?ÁÌu]"ó¬?äåûá§?°ëê^Øþ^?¦]ȳè™??"ÃÄÕY?ÔþzðÈ:Ó?°P=ÃБã?ÝÐR!y¼?¥ùw¡ŒF?¶ÄηĹ?iú®Õ?Ü~z0•ž?¥ê_~DŽ"?ÅoÿüB?¸Ç"'Ꞩ?ž›–ŠJ»?˜®<¯Vñß?é¯#‹UG?»'÷›¤Ù
?Ép ¦‹
?¼ªÓa+"?§â6€ð€[?©ëT•¾?è%Ôn'ëç?¾ãó£q?×WÃùòþB?±R¡\rå?²×~Ù.Aø?à¹=Λ?áù.(²_?²'ÐS/‡?ˉ—Zœ{?£Ú{E¢tÕ?ÀøL¥?ži|	qá?äúSdšÎ?©»—®þrÇMIXED4FGL J1853.2-0922c?íó³&;0¶À¬¦¡¿ØÉÀ9ËÇ;"TÀ;MC0×8a@nLÂ{e&@®qÛ®ï?Ò3Ȅh¯í?Óø[{¦¿r@j ÒH7?ú¥mL¿ïÿÈ‹ñ:?ïÿY¢Ò1¿î2ái<¼¿ÁÀÒº[Ü¿éâÅA¾q¿ïüí'hr°UNASNone!?âˆ	µq£?Í]8@k?ª^6ïÌ:?¯ޏ¥?Øy)
â¹?ÍÛ¹—9B?ÝVÝ5J¡?É£é¸üò?´l/q™?¶'"`"v?ݎ:.O?Æ­Úr–=?ß¾óÆ5Ú?°ãæÜdç®?¼£év5?¤®åÃ):*?ÙÀF®²|â?¯o­zá˜m?àÍX$/€?°/$Zí=?Éd$ºï?¬µ…2"a¤?ѳE%½Ã‰?­\í'‰?ÕÀ^wã?Èó¨6sE?ĝmìÜQ?ÃÉÙB@?ßñÑ&x»?Íÿ9å³?ÊÉÎ,j¹?Å´wùЀ?Ãø™l«­v?Æ^äß4¥Æ?äOfºfC?ʁ–\g"é?ÔW>J"w?°}3´?È%CÃC?¯äïþ1"?ߖ 'è§I?²5¬;7?ͯ¹ß'Õ¹?²ºTžm?×áa"\­o?ÀÀÅJªü¡?ÙFÁ}ìÈs?¼ÍÐrûMIXED4FGL J1853.3-2447¿ÌyBƒž=À&Û¦&oÖRÀ9ýìgpRÀ;µt1*Dw@ÜÓò0±@Ôa0œþ?Æ\ÜdokH?ÅҁGRÐ?ø8¸®1×@Ÿä6v?íê­ÞJ"¹?çßùÀë-¿éN¯{㦿ç–j€˜A¿ãi!—)|ѿ䍍â?UNASNone?ëO?%?Áa†{?‡{ÝØâ?ƒƒó™|?§p-?ÁUvæ#?îJ
(Å>?§ºnxÊZ?€Ág"ƒ?)•¹ÞÞ?§V_"¬"?¥Öó›‡tB?êÅqœ+?¨^è)àÔ5?š±õʶ¶Ð?b!ßÙþ?Á"üä9y?¦GïÁ?ì4?ziRª?'ºw¹Æ?™µŒ×Má?{8ÊhØw?·ð ÷½Ùm?ŽÝ•æ¿cÄ?èڒ²9?Àr7#?ž¼Ÿˆ:"?šž êp̜?Ⱦ!ÔÈf?¿_é…ÑKô?쌫b;?¼'#
(æ?™I¾¡G?¢°òsøÑ?¹KM‡ýwÖ?¸°6v.Æ?ä¬'aÍ-?¶(RÍÂJ?­pzC?šêÌ𑫗?Ó]m›}?´ð7g`¼w?ç9®ˆ¥<?¦o÷5ï3?®hW2eÅ?"õpA÷ë5?ÌIxŸ<à?£¢ædòt±AGN4FGL J1853.6-0620¿ç Gñä¼áÀ*èáÖIÀ9ÞŸ]'ùÀ;6â¿}Xñ@Ô¹¤{õÅ@ÁŒý©äj?Äá…@œ'h?Àí·(Ùº?øLZ·»+@ÿµ$¿ïþ;?ïÄÒݲù¿è‰áØT¿ß¥ý THØ¿ïýÈ[fX?ïB€®IUNASNone?êx*uÁÅ?ºÔ£}?"5?}68{CÞ?{w(1u¹ƒ?Å5¦'úùd?ºr'WæN‡?穪ýÞ×U?Ä-ûïWÄÁ?†*rÈ?ñWŸðà?Ï÷ágRci?Ãp‡‡sQ?æØ%ê[.?¯Ÿª>©Œ?¨d~\`Úß?šÝòKýӂ?ΆH½ø¸R?¬züüc•?ê؃p§ Û?¤ÖÅåØ?"<z$vfk?w{')éz?Â6b÷ŠÕJ?£¬YãÕ?áÓr#ÅT?ÅïâLL?˜ñ«ìf÷Ú?˜Ät$XÏ?ÚÊú¦Ï¸?Æ"ÆÔeG'?Þ¼N}šC?ÌôndÀ&ª?"Ø·–ΛÖ?¡GŽ´;Ö?àa ?́©"x¥Ù?Ü͊Éy?³lZ©Á?µåÿ3 m(?¤(:"xÿ?Þ²¨3e]?²ÎèT‡Ú?ät{ÂÄ
[?¶!´}…Ö?§7݌
?'ÜYD°WM?Ô0'ÞsñÈ?µÜ½Y`MIXED4FGL J1853.8-1107¿Ò
Z
´ëÒÀT#;z*À:TóRr"›À;‰¼9Ҏ@méLµ:_@¼7£~ö@æ|­_I?ç!J}|­{@'«¹VÎC@%ÎÚÄU?Ñ@|g¯'?ï{ÝáÈ"¿çÛ'£²ø¿ïà.ʖ<?í®ñðs¿Þ!§ÚúâàUNASNone?çz-¡µ<?ʾò Mï?·%K77¯?ÄF$,M;?Ƅ£ÞlŽ?ņÜÂR?àúü–F±s?ÓpñúÑ?¤YÅ^½|W?¹Ó>҉áQ?Û~Î&¿'?ѽL˜NÇ?ã·È*•R?±ÎtÔ©•.?¸në«kEw?¥ÂñùúO?Òt´ÀÅ
>?¯ÿ¯Ëz¶V?í'±@Ä@?ÂÄÆ¥ã¡G?\FMÔ:}?‡\(ÎL¯?¶Q]ôŽU?÷Ÿ€±?ãöýwåiÒ?Ìt§FÖS?È%¸ÇîQé?ËHâvF3?ÇþQX|Ð?ÃmØdtc?×@Žt';@?ÒÜ.ÒÙ߸?±Zg»@¬?ÂñiPóÚÐ?â4wØmƒ«?ÑÑw/ÑÏ?Û`ƒO¢¡ø?²´£äÅ>?ÄEß_mñ?®4Uy"B?Ú|Œÿ""¾?²«'UGÆ?æï,|Ïx=?×F4À"'?·T½-?¹{©êU»ø?Ñ#ì`]ZF?Ö¨q-"¸´MIXED4FGL J1854.3-3640?¶{¼šÇ×À0ZÅ;ËÀ:ÈPÓW*‰À<SAÞËÓ@$cb@.ø; ‡?Ó"ë|æ/Ÿ?ÔKÖãQª@yÀÌäJ@WIí	?Ðe0pá¬?ïîh(†¿á…ô¡'-¿Í']êâ¿îuLþ`m©¿ïüþy×ÝUNASNone?î!mSü'ž?œCR^Hj?¸äª½m?…yæF"2?¥Œ¸mkԕ?•k¹P¹Ä?'}+á?¢=Và|ü?EÈk|s?'óÓ3ߤ˜?™‰åAnÒt?˜7ÃË"Q?í•Æ•ƒ?Ÿ€ÇçõB?—‰Ë5ìøœ?v–4_X*?ªÞ± ï´?˜ôÚPü™?ëO5TˉV?•Õ/$Ž]Y?¬ª­q }Ð?Œãã Áª?·0þŸ¨l?)Š=D
?í(s¬?¥ãeÕÔ? º'Wؐ?•ì/ŠÿoY?¬½Ç'¤}?˜Çâ'@¸?ìO<ù':?¹ô]}'/¡?ªºýO²¬?²ƒãcúì¿?°)¸|Ù?­"+bEO?ì£!ò\î?¦ç}Ò8¨…?¡ºÊÅ5ª?"õŒÇi¯ž?¶•ää¼>?¢SbÒ­îX?æ¿ï 3Ò?©ÕVeÄÜ?¸½16?¤ã•â¼–?ȼѵcÜ?¤ß-K¸q=AGN4FGL J1854.7+0153¿ìñԜW—Ÿ?¾·¨£L˶À7ù$(Ô4 À9ßc¨F@ÙqóbbÌ@3‹Ë{?À^®÷yɛ?Íà*w¢Ï@\E˼+•?áh­éæ@Å?æØq
"=¿ç'ö?p¿å/< B¿å»bó_¿ê†È½¯#¿ðUNASNone?¼:á
²¬K?ÈDSêÁ]?ÄZêh¥A?ÄåD"üÉ6?çb㯁&?Í£Õ^äu?"`…£Xå=?¥BUÝÛ®?È°Â5çe?ÂS‹Úá"â?é0õâ€úM?ÂdÆ`aG?·ü›€³'?¤Ò*.Ò¦V?ÑþžùLT?²­'õ¸4'?ä[Ì?³Íc·5?G"¼ìÃQ?3h?'?µu2ÿS)?›â=wYÓ±?íFˆªÞæU?œáHÞ)ç?·3hï¶9?Îß!-w1?ÃýiÉXŠA?Ä_n:X?èB!W?ÐEªáŒï´?"‰.u/î4?–~gE&?Î/tz,0?È!¯£ØH?è!þD¾öË?ÇðòLt^?²Ì Òt?¡
—óýe?Óô¶`NÊ=?´€ØÚ+—ú?ã¬Ï''c?µ%&¸`
*?$MÞM¼ï?€½v§Be?»äÐØ'Ò`?¦dÎëã?ì'!až+?¦iE"g¯òOTHER4FGL J1854.9+4054¿ÀÌ&Vçÿ@0Â!x÷À;>D¬Ø:¿À<jV´A»Œ@þD<ÅÙ@Ñ¢£Y?É[~€äl¿šGÚ<Õ|?ÓO*_¥,?úZu—[Ѹ?±¹YÓ[a¿î³
=Ö$d¿æ@sÝGn?Ϲ¢x`¿é\n•à¿ïÿÿ²}@UNASNone?ï?Œ†Fç¬?›'kwÈ9?fMÅm?\KîL°«?•Me€»»Ó?}ÿbµÒ–?ï5jˆÉ#?™##-Q?px<s?t;
™?•4­É¶É©?–Ù""o{G?]e¼?'o×I«?t¬@&jË?v8œØ¬¶?¡'2,"	¾?ÁÔ6¨§Œ?îÔX'fµ?…]©Äf?t}o"Ù¬?bÁˆk¶ìÃ? 9§.—<ÿ?"ôI?íÓ16ȂÕ?©~½È"{I?x¨r§Ë(?n/m=á†?¯·Þ?p@J?¨¿¶£eV?íþюrw?±
qÆð)?'
²¥ W?'±SÏ©Ùª?«:q×7ÿ?®Ì¾I§=ò?큌ÑEi?3ÓÊ €F?›ºMÁy?}Ù.Ø.K?±ÄO¤?›»rð(É?ìBÑ_>æ?£Ó»ÚZUÁ?"§NŒJ¾¥?‹°·ƒ¿†¡?¸ÿ¡d­îT?¢úæ²ôUõAGN4FGL J1855.2+0756¿íQ<ï°¹@/«NiÀ9µÕ×7‰ÚÀ:Ž~ŸBP@!ÑÞÚkq@íê‰v5ç?Æ£Þ×fXÏ¿¥Nƒ_ŠBþ?ç§Làƒbö@±ؚ‹\¿ïчF°¾y?ïÿl'ù'(¿è‰î@dô÷¿ëž¾°nÈ¿ãëæŸ‡?Ч÷à÷§UNASNone3FGL J1855.6+0753?È´ì9[þ?½Íš'3½?~˜@u0n¶? ‹¸Ä!ðz?镔q"[?¾ób@oc?à3 s'ôº?ÏÛï)?š/Ö#¼?£û²:Ën?ÝùL%d,?Î÷ÈNQ¶?ژŋ\aw?³y¡Åv½?¶Y¾û7u6?¥)mù·úH?ßÐʵgͼ?³'¹nŠÇü?Ö8Ïn+›?²"¾QÓ?tã½Åîð7?bO¯"Ù>X?äÈä	?²+>32?¼·š˜i4?´èŸ®_
'?ˆ•=»ã ˜?©{fŒR¾|?ì·µõ?¸¬Jϛ¯?Õ)§ÜÛì-?É…8äx? hã§v?®‡/WÞ¶?äj¥ƒeXR?É_H­÷R:?ÑÄ´á"Ðñ?°'zÏö?¸s»—þá]?§K̵i?ä.Y8<?²¾ìwÀ‰{?ÁŠä_‰P?«ç$fà¶?y–⟏ÚV?s$˜3:±?ëj"ÞÏ?¬N®ñ´RMIXED4FGL J1855.2+0456?ïí5š°_?ösC>C1®À8(ܛvékÀ:ð)É'&@\àb€Ô@¦»Ò©†?¿õW°kP?ÉPx‹H@Šu¿Ÿ½ @Ê(K£—t?êœËbi¤¿Ù߀®'¿èº°ÕöA:¿ê¹ËhH¿¿í2Û>Õ}Ë¿ïÿ8$3»ïUNASNone3FGL J1855.4+0454?¨…±e€Fé?£+^™«å?©VŠ€k)?¨ýò£"d?ìâ<A"Œÿ?°èÿÃ81F?º­ÄQ†¸õ?¹·WvÅë?ÏzMR]Þ?À©»˜Ðyˆ?äË´!7æª?òµŽ0ž?ÄûËÔ?©ô'ÍÛ<?Ë1Ά°ð?±VÇOôÚ¿?ä2È;ðp?³T¯ÊQ€"?­ äȉJ?Š¼R¨¯¼:?ÅÎø$ƒ0æ?Ÿî'nÑ>e?è¼'è@4'?¢ÍdÃdè?W]"Ìu=?™'pÔt#"?¸ì"˜$\R?¶€­j¼?ë÷ÀÀÇR\?¹‡=l¢3ª?£ðx7Dÿ?©IzxeC0?Ñe§öÃZ?ÆßÃGpŠŠ?æm¨ÇVc?ÇQúDepÙ?¿wM¡b?¥¡¨1çù?Ь–˜Ö?´Ñuûbj?äŠàé?µ¦iz†É?VKOÚiá?uvÐj0ã\?Ì>YaÆ©?ªY…hýH?èm·M+#g?«DqøT‹OTHER4FGL J1855.3-0740?Ƅq¥<nÀgϽBNÀ:$ÀwSôtÀ<…
š¶@#²…£Ã@2ƒZ'ó?Ò͖‹È¿?ﻜÞÈwÓ@5ÿñ?ü€…S'wŒ¿Ó:9LQè*¿ÂùCbÖ9¿ãle¹˜<¢¿îUĝ~U›¿ïùzu$?鉸 šê§UNASNone?Äfôi&'Ä?½&'a¨!Ù?À'7KVü¢?¸U×eN†?æÁµàœ&?ÄW}4´À?Âñ±Üd"?ÁËÞû£yí?Ø['¶[Ð?Æ܇W8Ù?Þ,*sá?Å^ö½X‡ù?ÙÖv¼i?±ïÅÉÛþ.?ÒÏĢç?°÷¦ª¦?Ôd½«?°î
ðE²C?ÌS±Á6IF?ªv£é¹?ã¬'eʊ?±ò')?Ç¡ŸË?¥§õèO	S?­0픵³?¨ÅÓÕDz?½p'ž?·ÜA"MºÅ?êŠ~îz¡?¾·#O?ªÏeH";f?¶-¶{?Ý=Ô³c?ÍfrÊ;¼³?߉Ղd/?Ì*ì¬ê
?Íbòé?­UÎÍ.Ѹ?اo£¯zµ?µÚ‡)èLS?اKv ?´Ð³	¢Ù?¬¥
îA•?–™Û¤O+ì?æñߛ?·GácÇJŽ?Í¥2.?´wµÑm!jMIXED4FGL J1855.6-3603?î[kǵqøÀ0\'IðåÀ:ý6¤û©À<©"¾péw@ð$ÃXÚ¸@	üD~?Ò2µ^ñýß?êb–P@žӕ=ê@-}C¢—?ïÈb¥Æ!?ä̤S0ÿ|¿ØPêh¿;¿éÛÑý¹(Ö¿ïÿi'_Ž¿ïùõ÷h'UNASNone?á`é5?ÆwÍI§òU?Õv™[ӈ?Åc–…ñ?ÀqmøÎTÚ?´ÿºx]ö?×	–S‹dÅ?ÌE6üý}U?á/µ:g‹?Ë`³"p‡?º[üޖ?³"ñ€J
?Ùcìþ4h?³­Y?çj–?Ûlù?=úÚ?´-yhíAq?ÆçE§‡¡}?ªbµp©z&?ÒJ~Ú¡T?¨m·ˆÓÆ?ãè,ö>qf?¬¾ð'SL?·" Y½|?bͱw|{?ØofÙí‹?ÄSòñN·H?ß/LHØâ?Æf܋He?Á¤Â—"±¨?¶;:ÁZ?É¡
<º?ÉCÛÀ
TZ?æ"
¬™")?ÌÓìâÓ°?¼ÄP€º¿H?¸Y$Ûã¨?Ì{¦:M?°¹t¦"*¤?âÇþ™ùf?¸
x~Ìu?ÈhËKR?°)g8˜©?¹™…)G?óÇS	i?èÐÕæ¯"?°1Aì^?¿àAHʟ ?©CU¤©MIXED4FGL J1855.8+0150¿ë×Fà¡¿ÁvN{c"ºÀ8¢ _ñØÀ9º`Ðû/·@ `7ûÄÜé@ܙ®'O"?Èajh©Œ¬?ÐZãü>T@phÌ›?ýq¤Ýð`¦¿å‡´Nß¿ê#| âΗ¿ÓË ¥<%¿å^ÂÞatº¿äè,ÿèX¿ðUNASNone?¸Öž3'Ð?Å­,w—?Çxf$>?—ïH|åfž?ìf»¬5u?Æ1²Õæã?ª;:ܨj ?´@ÌfÃ?¬qæ/ú?¯‰ØÃfvË?ì•-ïQ‡?¹‡|%Ì_˜?ºÌðD\a'?¥Š:Ÿ¥	?Ĉê!á?«!¶	ò/?ç"]¼ëû‰?°h ¾Z?'³<kŠÏ?nÌ_Àã,?ˆpjð:šn?tÂ題?ïU¿‡në?~qÌæk?±|8sò'š?ÊqººHM?Š¶ŠC¤ë=?"‰rf7ä?íežÈW ?ÊI‹Ü?ž-Y<~Ô?§^p+?°ÒóàëpZ?³²ÇïÁ?ìô6»r®?¶Âkm è$?¶\Œø}S?¢€‰švwü?Å©ë¯Ø±?­}[a¯Û@?çÉóŸRã?±z°ý?b+ý~*[S?U"EÖ??‹g[v Ø8?~ýû	 cŸ?ï€6"š3ü?€Š'¾)ÙOTHER4FGL J1856.1-1222¿íg/!´8À‰"š|À9Èé<oÀ;¬‰RúxØ@nýúÂ("@ƒæœ«f?À±ÿ¦™?²Q_>e?ô'|æÛkÌ@5ՏºÉ?é2^ASÝM?ï´6Óѣ̿épÔH±¿Ó'C>™ê¿åÔcšL¿éºžÌßADUNASNone3FGL J1856.1-1217?ë'+5?²Dv~@à‹?q¼ÿÚÖ!Î?dôwv4"?Á>§Š??²'$±5"¿?é±ôè°ê)?¾Ãˆø®õC?q‡'ÆRh?ٗ3mn?ȯ#ש'?¾G±'ÕL?ëóQ‹¸ÛS?¥	—r/Å?Ž&˜Ú§·Ý?'¡…ŽYP}?¼  …,`l?£€ßæÎä?ëâ^Ø05Û?•tԊ¨²^?˜ÐÔz]l¬?zO–%{ё?º¸Ô ÂÜù?"qõÌ?ç‹ïî¡&?¼V]ÍÄ!5?‡©cÙFÂW?—ËÍÄ$¥?Ð*Õ˜"à?»Îíxé˶?â8öý´?ÇæVzy݀?|°h<{B®?‡]Cy'Ã0?ÚrÌq™[—?Dz§è;é?åm"·ÝHè?³"
&?¡qÒpšç?'²þóк?Ò÷€N2ײ?²sc›o<?æÄ@õq9\?©$XÀY£•?®µ4Y©??–"j²'9h?ÍA¯$σ?¦­-pâ§fAGN4FGL J1856.5+1735?à˜k׏É@R§¢pØ°À9¯0YddÀ;šätªÍ@žç'–òË@ù?ò^VÍ?ËéÖš9?Ïèw"KYp@Åã|;ºÁ?úqòxØÙË¿áZ΂¯rI¿æ¿‹€Ò"w¿åj¤ï81 ¿äªÅ 0!0¿ð?ïýk›Y:UNASNone?áÀræb?ĤàE`Ãu?õ¬'n?‡I_)<?ÜöѸÄØ?ÄÇJPtüE?äS(_ßRz?Èó?>üŒz?´)_hf?´À¸~	å?ÒOWfCUë?ĺdTé;m?åîc²¤N÷?®±­ÚÀÁ¬?®Æ™I@$ƒ?š×¦a-?ÐJeqýQ?¬]¼T̹k?è¥'=7w?§ûŽð÷Ž?§z²Ñ?‹©4Î0'¥?Ǎûˆ2?¥…JÌ)Z?ΰçi?ÁCÐïòÝ? õÓ%\!?œƒQ_—_ñ?çDŸï<ä?…Í>· Á?ÖðÓw`ߔ?ÍM^'Ÿ"ó?Ã['"ҝ?ÂòUõw]Q?ßac>¶ž?̆`Ša÷?ÝÀ&½Y:?²Qýdƒ?ºç!ŒÂ››?¢'>yAÈ?ۆߺÿà?±–2%føÐ?à[‰ä£`Ë?µ§ÞÕÞ¥Z?¶P	V G?¡¡Lu·W¿?Ù´é·¯Y?´úéjOD°MIXED4FGL J1856.7+0125c¿ï	i‰—ª¿à³PßìdBÀ7–|ÿ/¨À8Ö5¹ö0s@ÀÈGW@u üÏÊ?Ï(ퟀ8u?Ù&݄ªõ@MI€|'"?úCˆ¸Ë¸ü¿åە"d~?ïÈpçɨU¿Ú¬)žßԑ¿çÝÊD\P¿ïãÈ&tÞÏ?èëï<c]UNASNone4?ßñê)M?¡ ÓÔæ½2?tM'¥´N?'˜›®!?ï:¯õ>A?¥%ÞN?«ýïËӞ:?²dZr¬	?Í+[êGÃ?Â.Á˜€Þ?æõJÚ¥?Âð˜µTFd?º3³ƒ!?§Jˆ†Ä!?Ä.À:uÐD?ªn«´m=B?ç³ézò(k?°Þ<³Oþ?^cvʝ)¿?VY¹'ÜÞ·? Í5Ú*Îù?"´J‡Ô?îãú滋\?"–%'?z©=+Ô¢?§Çl.I?ŠÝ%_Šÿù?¢úI"•ñ?ï_8ð6‰T?® UþÒá?"ñ¬m@Q?™Ê¨§ å¶?Ñ{@ÿˆ?ÈN•,¢u?æª;Ò,÷Ê?È,ODÇìO?°-Òm˜_?œhõ–«?ĶÁô?«ä|ñâ×?èÚÄËw?¯©ÜØZ'?AK¤%Å»3?=ÃUƒ?¤j£ï«@'?ŸÊ¬[ÛK?îµØ;Y·? 
µ5±†®OTHER4FGL J1857.1+0056¿ï½¾¨'ü°¿ë-4¶ÀñÍÀ8…äÅøÀ:c®ƒ5ª@ ±—è¥@[ àJX?ÁºuÝ&â?Úg§cܞQ@9Úak@Ò¸¯3‰Å¿ïý*,ú4?ﯴޙ}ë?¦tûTŸ"…¿ã«ón!EË¿é-¯›cž5¿ïô‡'YY8UNASNone3FGL J1857.2+0059?¡[9†P»?£<þ€Qˆ¯?ٕ~†mÃ?х$Æ͞?â¿(|ÿc?ÒL¢ŠÙã6?ŸzaH¨b?¢Yüԅ?Ӂ'îíš3?Áƒgïä?åC˜ÿspÄ?Á.«mâ?¸ñvÎ4?¤Ñ®šóæá?ØSå®"Æ1?³ ³}~,—?à·ÞOoî"?´AÖXŒ•?Ÿ*w,DG&?€GYlk*Ì?Å)…nçÈ?£6)+Ï:?é¼Kšt?¤Œ*Íâ`-?"öµ"0?"ô'ô;¦Ÿ?â­À±Fŝ?ÒÓ4¤'32?Ùc/2P<â?Ó0ÁÄSµ?Š íe'Žµ?&ÿK¹·¨?Õny¢OÃ?Ç ÒHÝY?äà?xï]¤?Ç|Å%
¬?±BÈé/²_?Ÿ;ûÊ4mÐ?Ú%	ÊY*?·%§AÖl¼?àÅ!ýÖ¯û?¶›£>U?ƒÓϸt-?l'ž¾Ÿ ?Èœ:¸kJ?±íPzÉC?éKòi5ñ?²#䮈MIXED4FGL J1857.4+0106¿ïöq+;m¿êmjf¦'GÀ9¶)XüÀ;%ðÁž›a@ ¯®ôŸ¥@—á¸íø?Јñz+??ïÜ`w	L@h½=ã^?ó"ˆñ*Ð
?à'5Œ©Ç¿ìؑ[Ývh¿ÔbI€ýk{¿ÒtDöT0¿ì³L=pMñ¿äëIº^UNASNone?€D7F!$M?ŠâÃ'^H?ÅI㒥ÎJ?ÆR•eϵ?êlv>†ß"?Æ~*í?"ÑÊ@¼?¡Jô¬d÷?ÙëIÍÜõÂ?ÊÃÓQÔ¼Ž?âkÌÈ"̑?Éæi¾)?Éø" OZ?®´C÷ä?Ó­ËÏE?²WÄL2¤?ßUê'ȃ¬?²Í˜3±ëò?|<ÓÄ-"?fê5ÁÂ}u?åµÞét?º‡–ˆ~Ow?Õ¢;¹?º-³l~ƒi?mýD3[?t«\]Пþ?ÅMwEös(?ÂF/#ó¿?ꎥÔ?Âbãa/£?€<+5Ø
ü?Œ¦‡`( ?ۈÿ¥^–0?ÎóÁM'¯ð?áú€ï‡@?Ζ8Öò?ÀÜc‡}§?¦'Ú7ýZ?Ö,Š|ñZ?µ¿‹¡a?àâè$Š?µµÉ€›A?P«A\¢µ{?Gľ[¨ñÉ?睸þl_­?ÀØ%Ê®©:?гâÁ¼ß€?ÀÍUq)@ŸMIXED4FGL J1857.8-3220¿ã%y™ž÷ýÀ.¹<FØ+¦À:#õ|ï>èÀ<ëD‡Ž@Œé‡îv@†ó{??ÄoÒ Ì=Ü?Î0/ȚŽ@¢"›R×=@¥¦Z?ï'ãt®þ†¿â†?ʛD¿ãø]߯' ¿åóÂ[.пéâ6'¿ðUNASNone?î"Úßxå´?œYþ#1Š?‡—
Pµ?€æF©†C? ÌŽ±°¨?–¶™KïV_?îªx£"?ŸZ;|¡?}®~Žá?ŒGLtìŸ?šòƒNâ8?˜ÎB^ä?íEД54?Ÿ	RmeR?š¸ÕÍf¦?hÃuь|?®Qøší?˜Þe¯ÿ?ë+U@ğ?‹Ñ':E?¥óúg~ƒ-?z¡™0Hã?»«XÉD×ö?‡OŠ7ï ?ê®ì3YÛ?¶>­pÙ4y?ª×)ɲN?¡²)öXd?½	ƒ¿ñ%?°ÒŤÙKˆ?ëìÒe+íˆ?¶Î҅zQ ?«®õ2‡ì½?¬Ó¿Û!Ï3?²Áò>8"]?¯93Âï8?èï¾› t?°]x'Û5û?²'zX›)?¡zïd›Bä?Âû¿Ç‰Iž?©Ò[WïŸ?äc²f?Ÿˆ°B?¹I~¨Ù?"iØGš8?ÐØÈÔÈ(?›®?—:[ÖAGN4FGL J1858.0+0354?ë Èxp·?Óу€R ·À7òŸûÆÀ9ß:Q4¥ú@*ÜGéùƒ@@öÍ0 ?º¾Ä÷@hÑ?܆—^Uö­@!
hn~bÜ@dªõ°7¿ç¿sFS¡¿¥ÁÍBC‹¿à'" ÔÇ¿ê_@z¿îJ}ғ¶¿ïðÌö%ŒUNASNone3FGL J1857.9+0355?‹ÐWk­ÀF?/|Ð?ãÄIáÓø™?Ì/÷T	íj?ט遟Ž?ËÔÿðÝñ? =°'ÇΔ?¦þ²ZØ)'?á|•%ÛK?ÅÎ:svø¸?ÛÅä¿÷?Åͳ/Jxþ?±m&90Àk?¤/oÇG¯?ãsý¯)	?¶ ú>:œ`?Ô¼»¡Sˆ?µ2c²?ƒèº#:4?këO{á `?É{k
 Q?¦­e"ut?éQž^¶ë?§6#½?|>Ê3ËúŒ?t»ƒùö"?æѵÓÁ?Ç/8vWäÝ?Òál'VÂ?Æòá3Œ‡?ŠF|Xn–?—"c~èXè?ãíP?Töõ?ʌ>Ý`mÔ?×U%MŽË'?ÊpºÈhd?¥?µî&R?ªs±}ú?ä9xEOþ?º»­¦ÒùH?Ôå¸ÞƒY?¹l	™?c°UY	æ?QõÇ`$ª?Ï@ýAß?´0Ê옇/?èH+yÉ?´Hà»vvMIXED4FGL J1858.0-1052?ÙD¦HÍÀÙý6÷äÀ9ØB/OxäÀ;U/‰Z‡5@ý¸G"¤@dÐd1@	zg9Êüé?à7½½eQ@Y" ä¶?ôfxÚÝ1?èc]c2¿Øì#"¿ç_¿ž ß¿èÄ® 'Û_¿ê"•%–'~¿ä¤²Çë¼UNASNone?⛿GÂÑ?É%ÅX܇w?¾ù ìùVÝ?Æ¥A\Z¯?Ó
96Nèé?Åc§0êÈ?ÝÀ§
ׅŸ?ÒµAŸvl2?¹öY¬!d1?ņÚfà¬?ÛÁ‰
@—?ÍÜ	ü?Þ9~ôA×?²~KõÌËJ?¹«ƒQD?£f¤¡Jî?Û*ä°?²-êj÷­'?Ûhkyµ½?Ë°^u3çA?¥è•N]Ž?º®vét?àíA'xÑ?ËZë(W?×ß­§1?ź±í"'·?̝
ü[Êp?Éó'1Á9?ÙÒpõ$s—?ÈgÝì§*?Ѓ©a|‹†?Ðav°" ?Â9Ù?¡Ö?ÉzΈ
Ö?ã/´ÿYD?νÐÂïB?Ñ"Ž¬g?°8bW&m?ÂõSg
ÞÃ?¬{÷^{s?â³á%õ2?´K¬¿7Ï)?הU ‡£½?Õ]ôì•Y?ªrx@Ï6?Æw§èx
9?⎭듿î?ÕÊ]™À¦MIXED4FGL J1858.3-5424¿ín\´sÀ6¹øã¬cÀ:*z¡†ÍåÀ<jñé¼Çœ@µ[ d¹é?ÿyfâ?¾ét£@‰?ڛaðµà!@?ŠÒVy‰@öýÝ;?z!.N¿ŸOZ±&~¿Û9NÀ­YÀ¿çㆢ›öÁ¿éA6ÌD瑿ïó³KUNASNone3FGL J1858.0-5423?á*$»Ã‡v?ÅBÞ
Ø?ÖtTgØ£½?Æ+z­Të?¼Ýˆ~5²a?­Í÷Ôò½?âÇ
+rÜ?Ëú쥅54?ԉ1;%3Û?ÈÐËg¥‰E?½%ª™·?³m¨Û?؅ù?W¿ì?²=CÓ"?Ü° ýø$%?³Ld¥¢æ?Œ˅`7ß?ª¬‰Ðí¦‰?æNù_}?¢Ô­í?Å-œtÜ? p×îéØ ?Áš–f*έ?"Îئl€?Ï_Îv	
…?¿äúãX?âÌ]W/M?ÆN—g»%0?Ån¼+ÿç?¶ÞÝå[¶u?ØÒ<`·"?Ë[¼>_6F?Ýlö‡u ?Ì«jÃS'?Áš/§É™?·gÀ¦]SA?хpmuÇ?³'n1Þ_Ì?áHçßo3?¶R«ùút©?ÇÔ°!–)?®´TmÛôµ?Ü¢3Çܤ?¬âBÔ¾??ÒH¼©¶i«?°"tÕN?яG¹±?¥ÜjûP·¶MIXED4FGL J1858.3-1318¿ïUw©ïÏÀŸU›=À:`þԆÕrÀ;÷ˆy¶¥C@Ä2¸V@ˆÏa҂ï?Îà'&ˆªß?àFƒÂ—¿¥@¯-šlþ0?ó	ú…Õ¯?ïöëN˜ˆ¿Ñ‰¦ÝNû¿äŠ&_Z¿æ,zFíû¿ïÿ®k¸µ¿¿à¿Z=¹UNASNone?Ê좠Sr?¹€o"÷ï?Ӌyÿ(\?ÂЃ¡îŸ?Þþ4°®*˜?ù˜ƒM?ÎVÃÏ*Ӝ?Ç·O¤¥]¿?ÍUO®¥*®?Ŝñ¿í¸¢?áû ?ÅaM`8­y?Ý1"¦Œàè?²Ù¤æ?Êá®íO
?ªÚoTzi?ÕÁìüw"?°‡«Kÿ¦?ÇÛ¢R¥¿?šÄ­å
?Þ«ýÁ®®?¨	ä†,x?Öwf1þr?¥qÈ!ê³?» 6Ff—?¯3^~	?ÔøTô蹁?ÃõJXê°?âεbÖm?IJíÑ\Ý?·ŒI‹"?»f"g3HŠ?ÓQÔ¹UK·?˜£Ö¸Ê?ãeŒqñg"?ʓñ¨¾?Ð߄§fƒ9?¯Ï€ÔxS(?Ó3Ñãs>?µ…nž¬?Ûí\…£(Ë?µƒÒ%ß?¨>U*?…óLÑ/$?átÊN1*3?±\9~Qi?Ú Â,à´?°¿]®ÃMIXED4FGL J1858.5-4446?ïç–ØM<À3ì«Oœ À:vW&WƒÀ<X£Ò¿ô@²çÑ`x@ó8ÜÀ_×?Ç«µ¥é´?ÐLI'@ÃÏ,ù]O@ˆñ«©g?ïþaßîé¿àv'=\á¿âÑD£ÿ¿çg)ÚÄÝ¿ïüÍ{Hu»¿ïÿÚ@RÖgUNASNone?îà@ìü€?˜Y³>u?vÕX¬?rïktKŽ?žWí#oËß?–Kn÷=m?î¥j*@Ej?xV±p.?¯rÍ;­?'p߶ëV?šÅCrI?"[,_,×?í®½Ùٔ?_Ó$TÉ?™=Ûâý+]?²q¬À'Ø?¨0ãÑ
?•æÕ«{jñ?í%‰®XÝ+?ˆ¾À52él?¢ôT7P(€?,³³:pd?ª³摠Ð?€Ä½(ÓÕs?ì}oœ<ƒ‹?±óFÁiô?'Ûæ+~Å?'7hëà?·]‰'Î>á?°»È`G¯?ì_ˁPÖ?³^˜RŽñŠ?¦Ø
~Å>?ª]uò‹?±›<c¶óB?©u¡Üwÿ?ëK'°¹h8?¨rñۗCh?©›¾g"[Ç?š²Câípg?¸Õ"DëÂ[?¡Û"Â[L?ék}D#ps? SNï—v?´ß–?–ÞI~Ùb?ÀG›nŸ´«?—ö¸yoAGN4FGL J1858.9+3636¿à4ÃJåMï@,Êl¬Ñ…À;l–+PÀ<¡gSÌ/ï@¦å‡ƒÂ@ÀµgU?Ñp˜ïO®"?äý t-Þ@?ý¾Ý ?ü>t.ûì?ìÿ¢AÞÇ¡¿ÍÛF7Fé¿áò?£%¿èñ¡Þ6¬¿ïþ' ¦Ô¿ïÿþˆ0»ŠUNASNone?ã*.ñÉË)?ž†ÛsP?ÒcÙ_?Á9Èþèd?¾<ù
P(??²"ГW•{?Ø.1^ÐM"?Ì/»6;?Ûãì>Bu?É£ÿN)X¿?ÇÛÄÄ7r?À5å=±Ò?ß÷¥zÅ»X?³B1A°=d?Ñê—ÿ̺"?°}"pT¶B?Ì;…
Û'?¯Û…Ÿ®à?Üoÿîjà?¦YU^¿>?Ù?IsˆÛ(?§è…_ê¬?Ä£5sñ?œ.Yüíô1?Ü»Š*…B?ÂЖ0§$?ÖU*¢H[?Ã¥¹ý+(<?Éޖ·ºÅ?ºßÑiók?ǬO¦Â¢?Æ"ñDs?âëµ+Ÿ8?αœ'á?̤ÜKxú?ÄnÊÒ»h?ÕùÌZó&å?´©áû³??×Î¥à2Ž?·@ñøµ?Ò7Ž£,¦?µ˜éì#qx?ÈÂÿˆO´?£_‰è:€?á6&,ºs.?²í]'A?Ñ23âc?ž?­S8flÔMIXED4FGL J1859.2-0706¿æن]k…ÀÒiߗª¬À:M5fêåÀ;º©¢%YV@yc%¿,P@c8´|sï?ÓÝÂ=|¸?Ø\ø¾îì@	¦~â^.Š?ýrö6þnÛ¿ãÌÆ폻¿pjwÜÊ4±¿äÙÝ¡‰¿å•;ÁL;¿ä'̘ÊfÁ¿ïÿOÖ×èŠUNASNone?âGÁvÇ ?뤏}G?¡Öþlì>?"¥Xóæð?Ù5D¸°z?ÃsY4_ê?Ûuc=í?Äì¿,6z÷?¦;Aä?ÉÞ?£EQÚói	?àá‹/ôdk?Ãÿ²°Êk?â×SÛ89F?²Õ¥=±?±¶Ûˆå1í?›Êƒ"IõC?Õã¡g:Ä?°ì‹øÔå?ޜ\'	N?§"¹¾R5­?¾îÜl'¡?›ì'gd¦?Ù§ìbê0
?¨Gº¨Ø²Ñ?ٙ|W«…?ÂS~™ÛUH?ª›qgϱ©? ¹LÑåœo?ቊÙÉp³?Âèv1_ž?Ãè+s²e?»é"º²3?²FuÃ8Ó?²}ü3ƒ?è½&j^(æ?¿;yK?ØÙ{n"å?²ŽRå?·›SZJB? C\Hš?à ×øé¥?´"´·À?ÆΚöCœ@?¢<wÄKŽ?ÆúçÝtd×?°UفÍ0[?䍟Kÿº?² ,‡¡MIXED4FGL J1859.3+0058¿ï§é_niY¿ôðT@Éô«À8ƒÅL¥ËÀ:7m´Zæ@ ,½¡W(@N&&v‡?Ć<¶µ^?ÈÍî_ï~Ó@•;Ãûló?ý®àË¿ïÿï~Óo©?ïÿûB«÷¿ásœ¯ÎE¿åm_[°¿ç'sýþž¿ì>†ƒ<`UNASNone3FGL J1859.6+0102?®ò€Pø_?©ó‡×«?®¹¿ZêÊ?¶Nïƒ|?ì%<	=ó?»äŽtøO‡?»õei³šC?¸?U«X2ò?¸ŸPˆÃT?°]¢•¾.)?émiA"|?¼òI³þ?Â0W>]çD?ª"p"µLw?Ǹ¼^6R?°{‹ºfv_?养)Ðøš?³ÈVK
?°Ì·©Â?ðx6×!?±?*¾«³?Ž^zlE‹?ëÆaø‡?™ÌIîVLw?«œÛWm?®uuy´?®·ÿ1å/Ž?²'PY'K?ìZ¿9ú€?»ê^Ûq?¤ù¯ëÖØ]?¦m™é#.S?ºûWú'ص?·'äA$æÔ?ëPúýõÓ?¹p&÷+>I?»".ϲk‰?¤
R,Ø?Êb6úg?²{;ýG™?æ,Ÿ	3õ?´!Y:¤…?—ï\J3a?¤|?´ÒO¹T?˜itŠ³¦?ìÀjÛ¸oj?œVã·Ÿ(OTHER4FGL J1859.8+1545¿å±ŠÙ"¸ƒ@-ÙÝV‡ÌÀ:²€Þ·°ÜÀ;"''Û\@ •ù&rª@Î!¾–©$?Äk6D_«a¿´à!tK×?ó߄•%–'?ÿ«›úœê¿ï@†}ˆ?ï1KgŸV¿îû"‰µ ?¯•pkwó¿ÓûpcÀCÒ¿ÎÐE藃•UNASNone?ÀXLE0"P?½$ˆÂÔð?`¾·ðKŸ?`¤Pù``?ëÙm0Háà?½_WO-uë?çG-ëÂþ?Äë½[sKÛ?ˆ\7ø吅?"}¡ñuÜM?ЮÂhÎS=?Ä]Ƅ´/?á
†x!P?³EÁFBß?"Jµ,ˆyU?ŒÂ›ã¤>^?Ü G¼4׬?³^¡¹ã5ü?ëî®g˜%â?¥Ö}À>+Ü?k  ©f=é?^eò_·×?¿­‹¾åƒ}?¥Š$Ú#K?¸gÝöõþ?µzŸ"Ï=?s®ÏªXs×?rg~÷ÿ@í?ì˦¡êËæ?µýˆ©_Éå?áR´,íÊ?ÉàX`Ð`'?'KnÑ
?ƒüm\ ~?ÜêÐ;tÓÅ?Èߪ)ߢg?ÕÎhuV»›?±ÛP}ñÈZ?ž'¯`#'ñ?'7-ùzý?ä$6JaD‹?²"·åqú½?åX$ЀÕ?¼^nn¦/?†Û]Šÿà¼?'TB1[ÍE?ԘÛrpϐ?¼*W'ÀI˜MIXED4FGL J1900.4-4941?»Û 2áäÀ5½Å?9ѳÀ:öwZªpÀ<‰Ü°ožô@ëzPÔ@üÁr&?Ï8D,ï?×øúRAt@	ޏh"@p¾®üØ-?ïû¼¤`œù¿á§±ŸÊ¶¿ß[Á•â¿âg)¿ìêz¿ïþÕÞn_Ú¿åSu}°"îUNASNone?î¹KzŸ$ë?"2ž=[û?‰"È)¹‡­?\X1û"Ê?œ,_fË?Ž™¬è?"Ì?îÁ@Êu"'?š·)a2]?‹Œ÷·Í…?‰!vˆ¢šW?šŸ®"O?"¿:¤&÷w?ífãã%? §vñú?Ÿ'›o?z€?'aÐÇû?©Ðt£w?—¢úà>@C?íÿÑ(s‰?†eòt½q?É"VLj?vÛé؛Áù?°m¸â˜Õ?']ÅÂê8?í¥¾úëÝÎ?¢j¤Fmc
?™GhIj'*?'ð:À9NR?©\,Œâ?šù‹£Šÿ»?ì^'®).ß?´8UUÈü?¥é¼¬,?ªƒnî_?²Ju°Îlõ?ªrÿÖ(Z?êü‰ê`AÅ?ªä¾8½ê9?®åôV¢¦?éÖ¡K'?¹=´Šn€?£bf3ˆ%?èc5\öë?žú©Œ¨ZØ?°'ê\?'C6´½¤u?Ærj"òÝG?š§¼"gÍçAGN4FGL J1900.4+0339?ìxï#—g¿ÕÕ° CÂMÀ8'_3l>À9í¦Ý@ø.åƘÖ@¢=ú	F?¼üÛ2k71?Õ,áàZH@IS.Ô)@TöÂ>©^?ïÿý{ÁA¿ÕbàõΤ¿ãCàµ7¿é)Ùîm¿ío¶;ÏÆ¿ïýŸÝÂUNASNone3FGL J1900.8+0337?áÞ&È^? #‡‰?½?Ø
Ñݶ\¦?Ȏٱ%–+?ã
ÅSm?É\5Ø?±'Håº?±1EM¦¢?ÓÏ_j½?ÀOZ,¡Ò?ãèWÚ~Þ?Á3¤Búj?·Q†î6Íô?ª,ìÇ8ð)?ݬQ=pŠ?¸«M$Z"?Ýñó¢Ïx?·Ñ#"Кô?‹t._•»?p]vݒÑÙ?Āz΅è?žÿ1!UÓ+?êr)g¤ÌJ? A¶X²S?ˆxÙâ]M{?€JEö@á?à¦èµi6ƒ?ÅpùÔå'?ÝîgÆQ¢N?ÅlŠÜ9•?"ozÇÒß?—RÉ»Ð?×9ô-?ÆÆër|?ãNJbÁZ?ÆB§«'O?©fáíb?Ÿ³ûñ¦Â?à]ÙҔs?¾	HP?Ü#`ä­æ?½)C¨Ù?kXÛ¤,Ë?W,ŽÃm£«?É\AÕŒU?ª—{Z‰üR?鍖¯7N?ªÜYü=MIXED4FGL J1900.7+0426?ïµ5EJý¿§•TÝÊB{À7ù܄д¹À9‰W[0¨>@Û|_÷âO@tåÕ²Nœ?ÄÓ朁«?ÛpÇþ±Ì@@ õC
›Ê@"GÍÉ÷Û¿ïAhë{ä}?ï÷Œ"÷™)¿åœzŠ	ٞ¿ëj;=#¿ïÿöåv¿ïyöуóUNASNone2FGL J1901.1+0427?›¦êi¨¬?£‡ Dvÿ?´;Ôb/""?½?'™DV"?ì›U,=†Ú?À½™ë›fp?«5f§?µqˆ[Ê?ߛ5ïà8?Ǒè¯EAB?Üþ(ÿÓ?ÇaÍγ,?Á«Gn Ž?¯jû.[žf?ҝÁT|6»?´>mI¿?âFMz9à?¶S‹&~?y*Ðþ}¦v?bœb\"Ì?Éjï͂Õ2?©f9ÝÖ¼8?érîj^÷?©Î@ôŸ¡1?Šè›Ÿž?­IOj¦†?¼j²â|?Áº"'B?ì°=ÂO¾?ŽNLi:+?ôzôdº?šškmå S?ã{"¼à?ÊVûü݃ ?Ø]>.?Ê^®"±?·ùN
"·9?§ªª{þ£ë?ÒBkÁ*hp?·rá8³ˆ€?ãß ]œØ?·¥^[Æsn?Z–Y&¶?J˜X`Ã?Ð0æXJU?¶ÆéâF?çÚAq µ?¶#aýŠªŸMIXED4FGL J1900.9+0538?ÏeÓ¢®?ÞJ}ғ¶À8Kš2EÍÀ:%øÛH'@"ÞÏ®©@¤A"HG?ÈÞ½?ÚW<'W…ù@%B¯§ù@å3éf‹z?êàŒ1Ò
#¿à«µ?èM\¿è"³!*¿é"Ýr6~A¿îØú!ï"÷¿ïö[ ¸lUNASNone?"*sý`)?—cݶY6á?¸ùxqµò?Ênaý¡?ì?}b›?Ê464絩?°—ÁY$?­ÖüÕÂÙs?Æ$x>nê]?µ0Ì8˜Æã?ètNøFßI?¸"§¤?¶øšµ<Q.?£w@\«@?À)Å~ØV?§
j5x¿?é¢7ø¿Å?®Î{Êù?•MÂÐ>?uì÷›G»¡?ƈmÄ ü?ž"Áv {?éµµnŒO¯? B½9ì<?Œ£éK±?i<OS´º?¥o—¢ÕtÀ?«Åµ$'96?î6vá«"¥?¯"å#™?•u–BÁu?š‹gÈi?ƳyJ÷†?»Ô™¨eÂÛ?é§téêrƒ?»Á8§`?°g¤ÛÀP?šÜŒpVÎE?Àck¹{P?ªv˜"Š0Þ?éäκ/?¯C·ü8?svwwNÖ?\·ö¾x?ËÅÂ
ù_?§z†[ˆÃ²?éa GÍc?§»ä"M§OTHER4FGL J1901.1+0730¿ïÂí8ZÂø?ô9ÎÃG
À8Éw'ÕÀ:vnWÌp@J"á+~‰@%4åºÚ\?½ûÔ¢.=«?ÊBIP«éþ@©Ô#Ù?ø€''Þ@?ï¦~^Õ£`¿è¹Œ~($¿ãá"=‰ù>¿ä˜Õ^–¹?¿êœýýt¿ïb¾‰¬½UNASNone3FGL J1901.1+0728?¡*¬{†&?§r®‡2ß?»{Zz†=?À5vÖ?ë}éèïö¦?ÂêÁØç&?´Øs"é7\?¸F׋ßË?»ïø,ïC½?²í0>"?éæò–¯
?¾zOsÓé?ÅÕ½òqç?©û7[poþ?ÉGz:â1Á?­ÅgP6È@?ä8²0"Gu?²!búÙÌü?¢w§
Ù=m?"øÀEªÚ	?¶žƒµ?"Õÿ"?ì'θÏ?›¿íE‡?''"Ð]Ï4?˜ÛîXÕº?Ápµl*m?¿"õ¶?ë>ÿ¥?Áy[Øm?œÇgLRŠ?¡–g6»–?¹¼;<
™¾?¶<ñraj?ëâ=^24?¸ t °œ?¿-—EŠ}?£±7îIm^?Ê,Ëëȳ?°\þ=öK?åGdSÍÄ?²žôƒgW?"cÝ{»Ã?pŠ,Ql?ºHŽ
^?¡‰ž/ª?ìk'ˆQ•?¢¡5¤‡kOTHER4FGL J1901.2-7307?é
A©eÀ:"ŠT'À:Í*ô PmÀ<>é<o@FìËï?@7?Ŏ")uš¿¡¡ÛÇ*?Ü
ý¤[¢@F‹OSû*?ïù–Ys8Ý¿ë6¹ÀU›¿â¶ïö1J¿æ{þ¤Êû¿èíݾŒ˜¿ïÿ®XëTUNASNone?ïϛ6Ӎ?mW~òž"?GÔ7iÁ—<?:_'i²?u7êâÀ^¿?k­ÓSIâ ?ï³Uû4>K?}l¸h#?Uy{WÁ]?^7&¸F?€ŠrW?xEÁRŠ¯N?ïDv{ÿ¢/?"¤¯Í7«¾?e{æ+˼S?dÉIá#µ?"Á³¶rºª?ƒ¤µ&ËðQ?ïÐ¼à4w?dÃÁ
Ûn?W˜¢.+Í?<ØÊ4ûÛ1?‰˜¼ŽŒq?cÄ'·Œ?ïrîôâ7?‹Auìgp?\v‰&k?QfjÈ>ÖQ?µq°TB¹?Š)Ä_ðõY?ï5]E_}?"?'FÍ·?crè1܋Ò?rˆ+ŸŽ?–æ5»÷Þ?'l¬Ör?îW'ù»°?–iJŸËÛ?vÿ=NËXC?uç}º¯U¦?§­˜¼ëQt?"Âì2ʀã?î›ÈSÒv@?"ZnÌi&?qáªËL??_¶ vä¬?¤E€©ó?ƒwËRI/AGN4FGL J1901.5-2208?¹Pìiþ©òÀ([åÙäÀ:ä%hoUÀ<G‰ßrï@§Z
ã@u¦uJ/?Óãĵüý?×-KþSý@Ae%?ÿôæ³]¿ï—Jy Ö?ïüŃ,oË?œ0G¤í¿åß~ØÕ¿ã®ÈáÉ¿ïÿý¡UûŠUNASNone?ì5VÖrà??»0 ©$ÉZ?'#֓&?r~S–JÈ?¼è'r€H?¹ÿÈÖ%ē?îÂ!9OpÅ?¢µÒ s¾?ƒ+ʾ©Æ?ˆè€ol˜†?ž%ósn{x? 
qRe™?íTÞv?¡t®&I©?—®	uò?UËÛØzÍ?±§	Ô÷?g$Mþk?ë#hÅÓÖ?"*Iê)µù?¡ˆ+QT?ë‰Sà?¾UõÀa¦?'6á‰/Z?ë7…»ã"?»;§‡):È?ˆ|ÄT`Ýï?Å^<KÚ?Á™õ£ÊcÖ?º^'‡"?짽 ?·¤¼îˆ^?"ö ë?£E»p	üy?³`Ôk9¥a?´…¶Cæ?ꏾ÷¢
†?«us[$[?¢¢—§Î|?•»øF¯?Á:ÛyŸŠ?§ÀÀ€â^G?å½j^˜'²?¨RKðLz?«˜L	ëQ¢?—2*þö?Ñ!Á¬ïH?§ÊŒ3]-5AGN4FGL J1901.5-1112?Þ@î˜àJÀ;õ4v)À9ÇgŽ"'¡À;g2:å¯@Á"°Soi@"Ê<ϔ'?ŎºÈ"W?¿ÇñEÒó?ö®ÀWs"\@éz"¿ïh@[9â?ï{Ø»¿åæ8¨²f¿ìB­Yiþ¡¿Õaà89'¿ïù»þHoÛUNASNone?æ}–»À}?½Niƒ?…"AÐ`Ô?"ë@˜[?Ò\Åç?¼ªTtBêX?ë
Ì	-{8?ºÒÁe\óm?qÞqk!i?ytÎŒåW?ÃEÜO™×?ºLgÈÍJ?è·Ë«1?¬©»¢Cf{?¡v™ÎŠ+?""O¨bHð?Ë3z^s†h?ª;9G6"Ó?ì= Í*Ñ?•º$Ò½ê–?†,€Åû?pi¢‹{¸Ï?»TÔ–¶Õ?"xlehkx?ٍ¦
g¾ø?ÀÉ^Z~Q?Ž¡ÑA=Çh?‰F¥UådÉ?â¾¥´§^v?ÀÐSgäžX?ä–t-¤S?Ȟop•J?†yà9è¹O?–I(ݪý?ÖH£:ŠÉ?ÈRU.@ì?ßÚ1—Û1?²æñùNO?°C䈏¸?®#pEØê?ÜîG?²4'M·ò4?çhÅvõ³T?ªýþ¢K³¡?™[ÒTDQž?Š×KyÃÜ?Ï1oÙ×¢>?©þc°6MIXED4FGL J1901.8-0718¿èÈ\ù̓À}ŠÚ¹õZÀ:h'Β À<ª/@Kˆ{º
¨@$~d‰í?ËO¡¨Ü­•?ÜâÑ[|Óe@
&‹ýϤ@Áeý4ô~¿ïþ'A¶ƒµ?ïíjWŒ¯¿Ú
7`"j[¿âk8þNO¿ìÜʵ›X¿ïýÍáéOUNASNone?ÕæKŽs˪?¿[^`§"?ÌHŠÙôcÑ?º†´±ðI÷?Ûõo!¯?¾ù E?Ùݗތ‰?ÂêAV%jb?³LD܍?©ZŒ#Õ?৫Œðê?ÁüÇØ,Ž?ãl¥«ÜÎ?³¸'»&?Åùt?©0¡ÿé€?κSxxÕ?­Móþ¿ä?åüxM2|™?ãàkŽd?¿Þ&ÖjŸ?",74'e6?ÈÀÊØM?˜4X&{¢Š?ÆWoèñµ?µ|âÉS(?ÑmŋB?¾	n=Ë<ª?á³A@<02?Àj­{^?É)ÀF'?À\æ'Lî=?ºÁ¨Ó®Ç?·G½"G‡Z?æcu›¸ƒ?Ä%«Ô7Wä?ØzÛ¦·íË?µ%ñ–B½Ž?Й»k.)è?³èÓ!¿\;?ÖëhîèM?´<铢¡»?Û®¶†ÓC?§¶Œo‰?ËØ@ˆÜ2?¥]X O¦?Öe):¯?§±"§MIXED4FGL J1902.2+0448?çv/Äé©|¿Ë'^;õy"À8	Î^DIÀ9¥ÙUqK@+d²Lö@ãU9î8W?ÂJüèôJÀ?Ö–ä¦è@À7OøeØ@GNs*š?ïìPU'éT¿ã†áa¯H¿âÅîAÁn¿êX/ž‹q¿í]V½{öñ¿ïÿ§µ¼UNASNone?'	åÄÛà¾?±^ãǚpË?ª(oŽAòu?°ü$9s°?íÕ)ØõÓ?¸7Ññxà?²
Ú¶…½¹?²³Ê~[(.?Ыœ2rc?¿W¨°?åh֐|÷?Àm)š›€?²HUÓaµ?£ÒSâdÀr?Ô1
·>·?¶iº*.…?ãžxù»î-?¶Ã»)ïå?x
æƒBBW?aš‹É¯±h?¾ {FX ?2äîQÙ?ìÚÊo?žE55¹AÍ?¬³T¹gUª?Êf²¢?¹—ÀÈÔçñ?·…çH¹?ëқóè?Ê;Ã* ?"ú½{+-?š;C§÷5?ÓÚÃ:Qàr?Å°KhDs3?årÈw'©½?Å­Æf*?¦}™X¸?™Ü´e;²Í?Ö.-‹¦ã?¹ùØå't?ã‡÷'•Ã?ºË϶ñ?V ÖNÖ§Â?FÆþO#pG?ÂÙÞòØéÕ?¨ÜylæN?ë>7Ø"Z7?©S ðWÅOTHER4FGL J1902.4-3417¿êÝ9#"éÀ0üÑc4'¿À;³*dW˜À< îؐ@¼´B½>å@elÖÂïÔ?ÐÙ¬SœŠ?ޔ¹ËhH¿@½í@?ü'Ð4`YÝ?ïÿÇ`|Aš¿Ûò¯àWîÿ¿ã³ú8?ân¿æ-ô/¿ïÿ‡4<G¯¿î^€SwvYUNASNone?ëus•à×?¸Þ¼"…TK?™¶{³œÓu?–ìYLOùb?½æÄbΉï?¶C .WX?ëAH8J'?À"Y{ò>Ì?µ‹Ú±jZb?¶Ù–¥Aš4?°iãm,?°êåY¿´?ê4ýú°úx?ªGÿl3]?±%®ÀÔ8T?ž*`ý…?½2ajíÎi?¤)>ŒTß?äÂo»Ø?¤d;er$Õ?Çý¼],Å ?Ÿ~˜pր ?dz;EJÿ? Î<Ÿ©º4?é†Áƒ÷?¼ö"ϖ^Y?©z)0¾?¤(L†]«?ÅAImԑ4?¹–#"?ä,"šW?̓š9…:p?Í×âTžgà?É.'л€?Áv
Ÿ.Ã?¼t«M¡œ?ç‹ñîDkÀ?±1{0a—?º–8}0>?¥=\á0?ą.¬Õz_?ª¶oÊ/'?ÓÒãƒ-ؒ?§ÈÒÛôKÜ?Ô»Rg'²?±ft©<?×qÊRì{?±r4=ñ MIXED4FGL J1902.5+0654¿ì1:ᎌ?åãÆxõµ#À8ߜ‡Š£]À:q=V¢¤@þ½QYº@#Ï!?À¦cAøD?ÎBðj‹º@x¼œÓà½@-ÙçÁ¿îܼßCòÉ?îÞgߍCË¿Þns恩¹¿ãª?K¿êŒ?ÿIvÁ¿îìÎÊÔUNASNone3FGL J1902.6+0655?²—×àlµã?°"ÀkßZ?Äð#>œô?Â%E'.l?èpü4¡ûÆ?Æ™/ëš?¶!Ñ$è&?·É7ÊL@?¸·bz›?±ÂhÃ\Õ?ê$َQ<?½hC›?ʹè³L?­Ñ8âZ?ÈX¹'æՕ?­[Sîמ?ã;WnsG˜?²W}žÊ­?ÁiìöÁp? ã€7ZЪ?±·é.wú?Ž"ŽÎחk?én‡œŽbü?¤_ÏÄ/µ?¤ö`
?š±[\…?Ì4t­ô<?Áü騮=?ç±:üïï?á"§›?ª¤[ìV?¨IÅyyò?ÁdR\e©?¾/éQ½·Ü?êl¥Å¡à?À°F7Ð?À‰ð{ Þ?¤öœmÎ(†?ËDˆ†?±
ü9ªy?åaÛ^!?²¸Ìr}#?©ôO{Eú?'l)Á;ìb?¶ð¯£BÑ? å/PAå<?낥þÃ?¦^ÿÀš-vOTHER4FGL J1902.7-3246¿ãMž]<‹À0}»úëÄÀ:ÀÉÓIÀ<'oF	@dOÞ¾Š@ZR[íf ?à ð¥ïé2?Õ|8V1?øÞ<Pé'@^¬èÖC?ïü"ßphs¿ßÆí$ÒÈ¿è·ù1~'¿íÀ^à
AL¿¸¹÷2ú¿´¨¾û}å3UNASNone?í" h«:+?¿d‡Bm҅?¢c	"È1Y?ºo "sÌ?¥ZïäÏ®ò?±q,±cæ?ïTîÊ?£FNí´¼?Êå,
Q?zUO?"êÏq`Î?‹¡­f	‡?í ƺË)? X0éb÷Ê?™=¼#1?'x»Dè{û?°¿¯¼xl?šðÿÊ	ªÍ?íó"ÈíÔ?ÌÍ`Œ?u†""ô?gW¢³Wá?®%â°Â]¼?ú °³=?íÖ9Lr?²ºî.'…'?™œ_ ëÀª?¯eù~ÈA?¥Î?<Ñ£"?£A³Ébã?íB碪Ô?¹?hPWx?ž¯[@Ñ(?¬qªÛ²Ú?¬yØ95­k?±ƒËÕj¥ò?ë3€T€?§' ")Ò?¥}u$.?˜Ê¶#pþ?¼ƒ¥D%Q|?¢v$0òø?èA—m"î?±â*Ó¤h'?‹JT`J/³?Œ´rDo?ÍDý»O?±·Ê·<ÐgAGN4FGL J1903.5-0825¿²—èƒPpËÀüEßÞ!‰À:½……`ýÀ;!| dŽö@µIX8¦:@/ÂÝ_Â@zU_­å?ïÿûB«÷@
?h£Wˆ}?ý[îQ"ñ¿áô€oüè¿çF©½S2,¿ã‡Í¿;Ò¿î3Ÿ¿£n…¿ï¼ú\Rn¿ïif*×DUNASNone		?©
ùlãº?°è,Váh?§¯ø"YÄ?¾kš`qj?ìôPàÔQã?Á,·ÐÞ¡®?àAè
?ÒÑ'W¢m?«Ñ'J?½¦ø§Çà?Üy¨òk܌?Д{v‡µ…?ÛCŠ¬Ÿcf?²B÷]ódâ?¹å•Q©?¢k­rwñ?Þv¯ÚM¾Ð?²Õ2ø<÷‰?×߶x;j?ϵìò˜IŸ?±øIY?¬3P]'6·?ä3HCˆv?ÏÛý¤'‰~?©Mz8äE?®ô@®@џ?ªpTÙ6˜?¹Šù—Ö×Û?ìÄ'iGä"?½êhŸjƒ?Óy8-Ìt–?Ñp¹;¿?³_íuj¹}?Âéö(eϾ?ã×f:¾å%?ÐO
é;‡.?Óbnûòet?°¡"A0Žù?À»€eá?¨€õ1[?âè}#äƒ?²aðGì¢?Û´žJáÙ,?Øc %ºNÆ?"nˆñ,¨?»|@WÞä'?áŠ<™äB4?Øhû؏3öMIXED4FGL J1904.0-5925¿çCf×ý"À8­f8C=lÀ:÷ªëÑtÒÀ<ibXº¬9@¸=Qo@ò
ú/§?Ðmn-E	?ÖüadôÌE@ð#̍ã@°StÇ'?ïû¯8gOš¿ÞEý$ÙSC¿â âiD¿éíŽ
t¿ïÿçáüú¿å¨<b5ÕUNASNone?î»T'
`ç?–깏Ö?z£‡¤4?yM!Œ|Û? [cp@C?"£QrF@?î7€ö'Ü?¤N¼P¨¹ó?•»Êîf«?–`¼$ÖF?¡¹!ùhÐé?š¶Å?ÿ]?ì֋û r;?¢­Mñô{G?Ÿ¿øè"oX?"&Pˆ€-?±[¡î%,Í?ƒýûO?êÃÙ'ñX?'ú"%ÿR?§"¯4l‹r?'¯SÇR¼r?¾ß%Ñ)?ð%Dòž$?íÈ}<'	?£«šÈϯ?Œ[&˜ûL?…—\¦¿´ñ?¬h…þ¼q? ö—*hÕ?êozÎÊ D?¾R9É$v­?²b×Y8m"?´ÏÙ¹É?º!R0àƒÊ?²€Ã${Œ?êê¢u¶:?ª,°vТâ?¨Åp?¶¬Ø?˜¿`댲T?¼H42rÕ?¥J2ëD%?ã•w~šBj?¦r[V×Z?¶Ù3I™× ?›‹q9ˆu?ÓÄ0›ÿ%?¤íЫ=AGN4FGL J1904.6-2713¿ï¼äMê;À-tG䛬À:
Gĺ¯"À;ãW4š@×K±Ú-3@±eÆ-v[?ÅuNá|Š?¹"{?òÎ|Iýz@¨_iX^¿ÕýŽá"¿Ã¿æ<æp–¿è—Ý6§[ú¿ãÿšr¦ç¿ïY=SG¥±¿ïËBôqV"UNASNone1FGL J1904.4-2725?Ü
²p?~rôBz)?ZØSN=É?`œLÂ^?†~›º¦È?{§T‡?ïœ	»ÀŠõ?ˆ™ëR?c¸§sóQý?m~Tr‰¼'?"g38d<?"x¬ÓÌà?îpúÒÕ¶'?•›8®†á?†çÓK\˜ß?'RÿÕE<?£6]ü]Ôµ?'‰ÚÎ?B R_?¬iŒ¬èS?}ƒØîíSÃ?]-_?£Óà´­"™?€¿f)L!?îûïÑô¯?–ΰÍsØî?p$ 
.|Ÿ?eåURïpy?œxÝÖB=þ?•q¸÷ON¿?îßÞÖuÔ)? ð¿tŽa?{ÏÁ°¤L?‡»³Uõƒd?4Ç0Ý?(!ç?ëÙ¹–}õ?§GàÄoi? d毰þ?"LâªÜA?¸ÿÀLpLí?¢!›n "?ì+Î҂æœ?œ|ÔÖ O?"¨ÀšŽ?|l§p	cê?¹·‡§dï?™râ0cAGN4FGL J1904.7+0615¿å"€è?;w¿·íêÿ'ÇÃÀ8ãöíôÀ9úio/bÄ@*VgjÈK@¶ÒàD²?ӕ`˼?áDpù…@¥Y³Ð|…@º>èÉ¿ë*: bK$¿o*8sö6¿æÉäð°ä¿í­Ôï°ýc¿íÛo'C狿¿¸à[ÊÖþUNASNone
?¦³W‡…­Å?¤£\>¬l?Œ•Ų-8?'Ç?ü­?î"v"cÿ?ªeáNl¨(?¸'u>Æ?·yМ'M?µöÈ`?­-ºr^©?êLÐ5&?¹õvËI¦"?Àý†Pð&?©L¿«x«?¹Àсgs­?£ºˆâÉ*¯?舄;—
?°Þ%A/?¢Ð³Y…é?‰Ù¤,·Çl?¬³žHBŽ?<ƒcgÒ?íºåÕÃ}?™OXC=5x?Žžäw²jÖ?"¹Šï•v?ŒÁSÙI½?—âjCë'?ï¡´N? ¤¥åx~?¤ª«–šc?¥]äÞº¬?¹«"Ê«=?µ¨º97´?ëâÍ®ãÇ?·[)O`>?µ¶ë›Ü? r"ԍ­Ê?»åÚ©ž
?¥ŸœÒƒý?éçâ[ï?¬ÐªQ´3?'/‡ÁM½?p?uøü?®]"lÊ]Ñ?˜JAæ«û?íѵûW­D?™ê^+z[OTHER4FGL J1904.7-0708¿ïTꄇ}|À͔ÐÜüÆÀ9	wx¢À;'j¢5IŽ@)­RÞõ@3=??´ùÖ_—ý?×Òå XO¢@­H÷Q@xÀƒhTÓ?Ø÷}šµxr¿Ê!¯'Jq¾¿âHV°æ½9¿è6úh‹¿ë=¡ìNrT¿ïÿí )k3UNASNone3FGL J1904.7-0708?°NØlrî?ªyØ2Vuu?âg#_Mô?É]|ÝÌ#…?×%¤T^?Æ8K«¥	å?¹ÐÏó1?»œ]懀_?àzó;K†?Æ⹈¢Pw?ÙXÖVŸ…'?ÄÉÃ¥S.?ÏÞäì/?°qÁ>àKÁ?áè›ï6?³áôNIxÀ?Ê{~¯+û?­ÅT Tï?ÑÏ¢ÊV?£ð	½?֜;ê$)?£í'>Á€?ה¬@K…Ì?¡žããJÛ?¦»Ê¡u?¡}	"Ï'?ã+7¢iÝû?ÉsDt'è¿?ÖÒg®B§?Ç9n;ÍÈ?¦-"Î-Êé?­/p›sŽm?âq*•»?ÊFή×Ìä?ØWø+—ªÎ?É""Îó\r?½	?¯BxK?¨¸£Ÿ&ØN?åCÇ©ç|?¶™7þ–Ò?ÌlA'ècg?²Û!Ï2®?·²Ó³c?'J¬ù'0·?ÝÀUæ;ˆÂ?¬‹~۟šÝ?Üx=d ¤·?ªh9OWBMIXED4FGL J1905.2-5120?ïú™ŒŒŽÀ6ï6ÍòfºÀ:E£_9MÀ;ø(/Éò'@4êv*ÿˆ@-ô!¥l6?Èg$|a$ˆ?Ìj¹ºv^@ä ¦hµ@ÿ¬ãÎF¿½¶˜>6Ö¿âL¥)ð"R¿æR¿ >yb¿æü`£®ÆR¿é›r·­¿æ£Á`]öUNASNone?îãFÊ¥çA?œ¦2úÿ'?}^—mKH?{Ü{yD¥Ñ?œ?€Ë ã?—ã`ù?ï-Öog?"YÈïï?{ÕZRmsi?~xð	Èjº?"OۈÇý??Ž~ߐ1e?íõ!ØËfN?™GI6}w?¦¥Á|(ô?†ŒÑá¾ß?©D9êä?"Ð…éä_»?íÓnv#?ˆaÔÐ42?'Ø=Ëþé?lÔ÷ê?³{UH.?‡,Fø…?ìÓ¿Žåz]?¬2Ïvzy§?šžc	†?'"¹¤,?²Ý[ñZ…9?¦­*õ:îØ?í‹àýlŽ?¬Z3rá.?•6ן½Ú?š|¶}ã­$?¬¦"VÄæW?¤ç҇'Ýï?ê³jùH*ç?¨½æ,©³?¥@ÖT¢ÿ?—Ïl¥ŸÖ,?¿ä‡Ç'®Ì?¤7æ¹B?箛ø¿9?¡B¹'ÐÒ?§È(~Àã?ƒ2—§r?ËS†i"å?¡œy[¬;AAGN4FGL J1905.8+4942?¥ÖËÈ"À‹@2'0aǛ5À:õuD× À<Àêù¾:@à¼z-Ä@»|Bp½Ø?Î\^¥§ÄÖ?é§)¥÷ß@-9–ú'è@÷bõÑ¿à±`ôâk?µ¾ñlê9¿âi`Á¶Ä¿îª5]¯Þ¿É
ý«è¿Ô®)s–БUNASNone?픖5>®Å?®ÒB¸¤[E?"¶Èì|òB?–ß•C¡ÿê?¬[83Bå'?¨•-t
‹1?î#ŽìRµ@?°gGX?œyîOö¯Â?¥úÀ¤ÿ?Ÿ4"CI?žrÙU5*s?êÉÝSؚ5?«C»¸ºÑ?µ'/øC²­?£Î㹉Š>?´.åh÷{§?¡c1gq'?ï'_Zp?€XM{3T"?…ÿí'äŠ)?upó6øs?'O½€Ê,ï?s#ÕèÂ[6?ëµ7¿ßÔf?¶>Œ²Uá?¤å‡Ä/s?£òB•š¿?·ã~WÒ?±bx]f?êãÛ?ÃrxHø'«?µ›.•ÐÈk?¿C?Û7HÂ?³L
'ö¯l?®ëҟÀ<U?èeYîU?²hÌ+Vå?Á­h1Ë?­V³]íÖ?½º
Æ`)¿?¥Jò§ÞÈü?ì¸6+T[?¢|§ïwæ?£f+'ªí?šdzÁ#?°‹9‡‡´š?•œÑ.ÌXAGN4FGL J1906.0-1718?ïÐøƒcøÀ%æFÞ	À:ÙÒÛچÊÀ<Yíð3c@
æ®bœ@#5Y~ —?Ò߂\L(?ã›bý%Z-@x~a.ï@mMÅ×U?ïŒ3Ÿ¿£o?"2ޛù' ¿¼ÄfKäZ¿äô>‹$¿ïþ
A¢a¿¿ïcoqY	UNASNone?èò
Š=lX?¼5‰0¸&?«wÍ)?¢Ï»äy+?ÅZãàÕ?· "[W²?ßó5ƒçÍü?ÊÉâ8çª?·äò0ØC?³ïÍÔoê…?ڍøûó?ÈéªÖm?è¨S#q&ç?®éú©Çf?¶'ùŸ
>??¢$7¼¶¨i?¶¢¶EC?¦kÛý3 U?èHˆsÆ:?ï£®žÎ?¼6‡¢1~ä?–ËsC_u?ÁϚ=é"?•°æ&
å?ã¥P'½Ø?ÇH3J…4?¹ —–öVR?°ÍEzú?Òm8ötC§?ÁÊRÉübè?Õsq3@l?ʗIc²h.?ÃåÇßA?À j2¹Ö?ഌÕnˆ?ÌC¾Y3«?âÜ}ÄHfC?µd^nˆ/?Âë¾A;+?«{ìÜøï?ÐÑ%Wä~«?²1ä錾?áqinzÿG?¬v½¯+?ÅÉ{Fûő?©"Æàkér?Ò8oŒ©?©Ý¦N]ÛþMIXED4FGL J1906.1+1651?éxwHZ.@͉âlqBÀ:¦"Cƒ…À<x­"šB@ Gq=ÚÖü?þ¦öyn€ç?ÏjÜs­?ïmi?^º @\¾Fø@

 •L?ê}K…:¿î›éÕò|?åxUFƒr¿Ò&Æ0<‰¿ì³Éá`È¿ïÿÚ €UNASNone?Ä4ú{º>2?¼Sâ7ÿ1?ߏv/‡,/?śØI`O?ÖV'ˆÓú?é»áÔ,?»äO†Œ2?¾.¿—@_?ß/uˆ8?ËC3Õß3ñ?ÙìQcD?Æq²{N??Ój§íß÷?±Î1ê/t'?ߋ"ØíAŒ?´Æh'	9?ʦpA±{?­8ž›ÐÅ?Ò	¹;¡¹?°Œtà˜)Ú?à2Á·[?¹½º±Ó]q?Ë!†å"K ?¯ð ˜d°ò?·‹ÝÈúX—?³/°%Yþ:?ßwð¡0Æ?ÆM–Dê/?Ú¥ìÛµô?ŝ#ÒB, ?¨•6Ù<'?´'Åío
£?à壇Ñg‰?Ï«c8½z?Û"£¢©?ÍFàHCu?˚/Ÿ2"Y?±Üæ?º€?á,>"ûX?¸²ô?ϵÃf½Ì?³5(|õÖ?·;˅•yÑ?¨6"¥í?äÜäX?î>?©X¨…£?ÐwDmu×Ñ?½ÇÚ#jPSR4FGL J1906.4-2001¿æ¬»"ûÒÊÀ(VÑ|^ö0À:e-Ž¯À;»üߺ[@隆~‰É@D[Ëر?×µ?¿ˆ—?ãuf´iÿx@`†R•@ðÒæl?è9€õ]县ãE;©#zY¿à†Êßâ©-¿éoÿ¢.â¿íÈ1\™¿ïà'¢ sUNASNone?é79.Â,­?½ÇGxuø?"0ëZV«?Š–,2Ö'?ȼýÙ¬{–?½	Hh¤".?ê'L"¿Pt?À¸"Ö°s?¨‰¹QÅÅr?¨êKìEA?¿0¾±"™ª?¼+ ©?å-þÃzT?±—§2%Åv?·S)®Sª?¢
a£š4°?Ϟpay[?®®OñöK"?âYº^ÇG?©y6ïø˜O?°µ}(%·?'RÒì¾³?× žìää?ªa9³œ@?ä™ÉXГ?ÂWÜ/˜?¦Î*§ÀÆ&?¡¸¥`¿?Óò§û¶t?Áj#™Q)?äðaäx]?Ê7eýŠÚº?½®qu–¸œ?½hüT
)‹?Íg?´öÂ??ÆuíL…P?áLs'5*?³µû
_¶Š?À™øѯ×ì?¦Ý7J'k?Õs©¶?±©ô–Ñyk?Õ«¦VÁWÏ?°NQ£÷ñˆ?±Ò¤¼E<¶?¡QQÍÅH´?âïØ<íq2?²`±ù²MIXED4FGL J1906.4-1757?ìïî¡¢–\À&™
þ`ÏÀ:_¦FPFiÀ<dÍ	2¯@MÐù^$@'ùºk¡9?ÈJŸ¶i3?Ô"Ãäƾ–@†ý<× ä?ûRŠ.A²?ïôÕ?/c¿àÞ1yÏϿܗ|=¾&—¿áDêÜ0¿íÖé¡éÜ¿ïÿÞ§À£ÊUNASNone?ÑòoøÐ$µ?Å©PÍ35H?³'Ghz#?©†ÒÒÏ?䔟"*Þa?Æ7Ѩ~¹Ä?âPµÒµD?Ê\㠏?°¡óL(Ò¦?­>iâs?×6‡8̃?Èaå£2u?å2C#›?³Ê8·›Q?·$Íôëb?¡b°¡¹qÓ?Ï£›÷¨ÿ¤?±ï'±|?åˌìô? ?-'_h›?¹îd[&ö?'*]DÖS?α͚œ?ìÍ»b¬?Íð+¬V4À?ÁÓ£œûè?¹U§ã™=?¯¥XÌ?åY@|9?ÃÍMêÞI'?×'YñÒ¯?Ê¢…	®nW?¼ü­¿Z7H?º"d—óëä?àÌۛÏ¿?ÌXÇó°L ?Þé谜Ú0?¹—ݽõi?ÀKQw–å_?¨+KX$ Ÿ?Øðn"ª"ß?¹B=>XÁ?ÚRcl-r ?¨áÞ¾œ?Äe¼zø¢F?¢IŸããÿ>?Ûz¾VV<¼?«>'áeXMIXED4FGL J1906.9+0712¿î¼ÖÒ+©¿ÂöÈHٍ¥À7Ÿž;¿É¯À9Š*^x[[@ }øäWØÚ@˲5qÑÔ?µ®úS?ÉÙ×¢=×ý@A#=ó?õ· ¾œZ?í)#øÁG¿í*ÃQ#?Ùjä$'@¿ãýl§É¿êŒ<ït—'¿ì*úIݙ¤UNASNone?{/÷ûâׁ?ˆŸÕúœ3•?¾äþ-(=r?Ä<
ôÆw?ëíJ—l²?Ą¾Z!K?†x³¯•:'?—h۞'Jò?ÒßÂÀ%ìÆ?Æ`80ëQÀ?æ6;Ñ<s#?ÆDË8DŒn?³¶¨ØðªI?£}'¶œ	?×?û,‡t?¶/Pðv?áé-N¨ë­?¶©Ø¥è?RMe(j?>[C6À²¯?¹€&m1n¨?¥çQh•z,?ìÆÔ–±?¥öçG_UŸ?rÝǔ©BÎ?""ôqž6?Dz'‡ó?Åö€n?éí£ÎôÖ?Æ%þj1T¿?{‹€AÒßì?ŒÓ.í|?Ô¦
øùÈÑ?Ë«rŒ0ò´?åuãƒ6o˜?˅%] †L?ªüÀ]è8o?Z1PL?ÚtãYšë?¸Ù¯{ô'9?á%«¨Ã?¸oL«¡¦P?0¿ö£I¹²?#÷¬Jj݊?Á#Ûq«>?µ2ùc,ô?ë´ñ%
•I?µ4yÖYGOTHER4FGL J1907.0+3556¿ÝÞŠ¹Nb@)A?À	oëÀ:؝@îÙÀ<^'ø»@Ò¨'Y.E@žº»RQ?ÐA°dmF?օ/IŒ;@$zü ¯?ÿ[Ô½0¿ïy‹Y?ïó}ü…!¿ä¶ùáØ͌¿è©H>]¿Ü2-d<?¡¿ïÿÿ" 5•UNASNone?í®QÛ{!›?¥]¤ Þ²R?$ϧ-?€KZ'¦|?°hí«ôÍã?¤Ö,՝—?í ÝŸqº?´…nO¥	?œŒ¥Ã³}?¡)&MÝß?°·Ï¡;Å?°z퀐M?íz¥¥7ÿÃ?`°uÒ_Ì?•à/3n?Šù+¯Äí?­Ôµ"?˜T9®›‹?ìˆT®X?wO£Éw? Bçjzñ?ƒ›'êø[?³›ëÉOÈ?‰ÍÜèý?ëHQfé²Ð?³Î‰µQÚ3?"¿{R1®?Œ_½û"¸d?ÀfÊø"ÚK?²½Šhèæx?è­o#ú02?ćJƒÿþ?´¾5Q½Ú?¶ç\üøg?Ã@äVA?À\|•O?êí1C™Ý·?©Q"^ÍT'?¢£ˆh–X?"û¦"?Ð8?¿G¤!|?¥Ú‹MçĔ?çeŠ›¤á¡?¤Uƒq}T?±x°û©çÂ?ÜÈ@Á©=?É­}ò˜[?¢ˆPÌMçAGN4FGL J1907.7-4037?¿ÃCÙk
7À4.gù
wÀ:€ž<–‰DÀ<*&i U
@šã	û'@,ý>" 
?ȵ&gó¯:?ÁŽŒ	äw?ñM¿¦sœ°@¤êÕeM¿ÜÌ~VG4¿Ã¬Ö!à$˜¿èìXþÉÊ¿æ­´©^3¿ïùà#kÀ?ïªóɐØ*UNASNone?ï'Q<¼?‰I0ˆy"Ó?a²å+¦""?\ä^ƒE ?‹n-¥Ã?ˆjŽGB?ï~5i]*—?‹yueF{›?mƒŸåi¢ð?tÂ/ù	œ,?‰½­ût?"ö9šGÃ?îÝjÆ¿¹á?Ž"æîÂ?½ ì?}bÚÉòHN?›ÉH›À´g?ˆÁÙy€??ï´õ`Ù?{dó
çC?w(	‡ê?\ã÷äc#‰?—ß|€BÖJ?wMÒopʜ?î³ú"¹¿?¡	̈́éÅg?sb5¨†,?q0dÉóœw?¢[¿ÌÆX? t¿ÙÏ^?îE_ۇÑ?¥îà֖€?ƒ»ð_?'pԏ)w?£Eék?¡ph(ûzI?íÉ.¥.ù?œeV <\?Œ15Bš?"÷½?¬`Ô*_;?˜01v··?í*8ýïÑ×?™Ndæ)WL?t)§×•?|EòÅé†?²'-§Õ‡á?•ðìnŠAGN4FGL J1908.7+0812¿ÊôÀÇ/ÿÍ¿³÷
þp]áÀ8ì8¢Þ½À:™8JÊ)@'Sæ/@'D¦">?Àé+}1Y?ÙmucÚE@VºI<‰ô?ÿP­µ"¿£Ñte6¿çUá"oA¿äÕZXTU¿êޚú—
¿ìtVÿk/¤¿ïþ=RpæUNASNone?–ø/F׏O?™¹M륒è?⋢ÑâÇq?Ï-Œ%ùÊî?Ùy7h:ë¨?Ύº°5?œªÃŒì"?¢}Æ©mT?ÚÉô•¾˜­?Ä}[_ø
B?ᵰƱզ?Äñ–Ç0?­ÅX–ó`°? 	¯FÎb?Ú\'í…©ù?¸GôJ}Q?àõhÿÀ6‰?¸øÛL?{ø']ìÝø?`c•×eR¥?Ò+ׄ`ÍJ?¦‹€AÒßì?æ²#9|3¾?¦‹ÌÔ
ñ¡?''†"ïÁÝ?'—Æ}Ü?ãd
ˆÔ¥^?Ê×ó1—x?ئ¨¹z¾?ʞô`ÿ8?"¨]Z7Ôº?†eOß)?ßF
GÎî?Ê5"	b?à
Yf½h?Ê•v5´?¤ú|0É?—^A¡,'a?܅ý#¤?¼Âv
éç?à|'f5Ù?¼U\­ì$?T	4{lØ?@Ko¹À~Å?Öl1Ea!ó?°­jœÃÿû?ä¿âÃ{Œ¶?°ªŒ¤Z(MIXED4FGL J1908.8-0131¿á./èZ;ÀHðÄXŠÀ9,­m‹ô•À; mµ@æ@(¬ò'Ø?ÿè˜n#Ê?»KVët-?ÝÑÖÓ°@ ¸Óñ"<?ýÍBŸ¿á9|žCU¿ Î˜ÃŸ–M¿Úié=EÛ¬¿âÑeéŠs¿ï(¦G'þ¿ïþ#A"µUNASNone3FGL J1908.8-0130?Ÿé.Í0ì?Fî"q°?î! v/Ì?¨asS²û?©†>–…?¥–ê³T»?œ•ˆ@jy'?£]~ð§Æ¤?åïN»`$?À‰¥¨%?ÒX
p
?¾Dó5Rƒ?£`¼…U?—J*bØ{ý?êàcàz(»?©ók¶Ì@?¿L'º"öŸ?¦(›äÿFè?¶9Là€?'–—>rù?â"nËJý»?¨k…a¸³?ÕvޛMÆ)?¦¬wO‹?€b#†â?v™T…Tq?í»~~5:?§09@¶?°Ëjû`.?¥}oZLS?Œ5b(‹‡?'"/g?æbtDS¿?Æ/ÓN¾v?ÒYn›¿
Ç?Åð™MÌð?'&@ìn?‰%í!€>?ìY³1?§rA…=Î?¸­ºCsë?¥u÷Màо?œC
²kc?}Æé"?ã¼ÎÒácÞ?±SP¶±{?ÖÂ1~äGÏ?°ÓáÕºµˆPSR4FGL J1909.2+4646¿àƒ?íx5h@0.3ðÀ;7hWØ.*À<Ö{@›å،s–@UŽäÒ?ÍÉ4¼Ë!ý?ÙT%ò{@¼éåâGˆ@?UÑ{¿Ì?	U>K¿á͊,>Ll¿Õó"\¿áæ—䍳²¿ïìRnaÝk¿ïþß06)UNASNone?ìí‰uµ
é?®úDz¶¿þ?ª˜¸îÕ}?¢Ø‰°¢²?§ÏëÀKî?£MuX
œÖ?êþ?>6úò?¸Ñ$¨KÅ?³">HT?ª´¼=fš?´‰ïîÀ¢?°é·×+Ò??ëFBöZöØ?¨ÆªEüH?±Ê=ö? "ØÝËN?´̽XF°?Ÿ"w£h?뉂‹Ç/:?"X.¹R§?±ba㹒!?Š±Ä¸Ëî?²Q‰¼U&?Œzýfåý?êd7ú ?´#‰ fã?¸dƺJOk?¬W‹‹œ¨X?´yyq¦£}?¨=ÖéF?åSŒ½pÁè?ÄBÏ_›"f?Æ¡r÷zË?ÀÍhÞ»·§?ÄZ$}–?·‹"p³?è
KC±kÙ?±æ[>­c?½£‡•F^ð?¨óxæ¤Aò?Á&—!"?¦}I:ˆFs?åÒ™ý?©#ÏuÆ?'î0Zø?£bMéGÝ?È>>ki?¤W#oŸ4AGN4FGL J1910.1-4704¿©êß$é†À6ŠZ%"À:r·ÔCéÀ<F·`Sý®@8h§3`@J4CÔk'?Óà]7é{Y?åH-€Á±f@eöº «?öÔkçÛ¿èžç·4¿áw—±b
;¿æ¨¿aÕ2¿îì<fd¿ð?ðUNASNone?ìt­kÞul?ÀñÀ!BÅÍ?€¯ê*	°?¡'nN­>?ºD—Z`Yî?ÀA&› /
?ëÿƒ°úo?¾Uvæ!˜½?±16³í?µ–¸Î‡â?­¥XÆhû.?«"§c }'?èZ®®"ô?¯É»­¾à?´|	¯¹é?£}ϤóˆÜ?ÄWBéÖë+?ªÃxy9*?éñøY²<Â?¨G®¿ÂR?°4È£a2d?˜ÖbÅÛ?ÀºG†sÄ?¢\}ö¤,]?êt9ÑïÅ?Älu'0ø#?‹
Ç_0?•Ä¿)yŠ«?Ä~lH
ñì?Ĥ<WA?åàÉj'ø?Ìò+Î\fU?ǗæÂ}yº?ÇàYã\ly?Ä –Ùæf?¿ ÙÌ1ê?æˆdßÂa©?²1RI@>H?¶,,îEy?¥]}ó@—?ÊÛVjc!?°×Ã!²•?⪃­…E
?¸Aš©3÷q?¼ Ó­f«?­*¤^èš?ӂôð
A?µ˜ µT¦šAGN4FGL J1910.2+0904c?åQ
ìíÿw?5ïò<4üÀ8Dß-!¡À9òŽù,§(@!;êH³£@PwDŽ¥?ÀZyɹå?£¯a#}Õæ?ô0ÓÊ?ú$ÉâοïšG©â¼ù?ïÿd™ÝŒ8¿åµ)ã(Xå¿Ø•ýB`wº¿ëH¸ ÅÝſаh¾‡úUNASNone$?™ýu$—?™¶…bZ1?"ýZ=¡Õ?¦ß´é¨»ü?îˆ)…=Í?«\}Ãõï£?¨;¥bC¤Â?¯øgá]0?¹%£p^Â?¶øàúFÑ¢?ëW¤5m¹Ü?ºý¥\ÆTŽ?µ.Àgü£?¡¯IÎè÷I?À4ǒ¦5^?©ç^%R´~?éLö©Tç?®ˆFDŽÎ…?°žÏ5‹;Ù?'ùh6J>è?¯¦8ÒhG?"pöډÆ4?ëñ™(kÀ?žX˜??˜{¢ï å¨?Z#%>=?¡Š¡'?®åµ5ˆK^?î#'wØÃj?°¢fj? f®kÕê?¡Ãå…Ïd?¾Ï€¡é0?ÀRµPý?ë$i'{ÿ;?Àm–Ó¸ñ›?µBªï^E{?¡P$?+bO?¾¢šÖýʓ?©	y)³¶?éƒWFý"??®™ñø
>î?›,IûoÏ?†oDÌܾ½?³¹=B¾‡? °tû^?ì°.õÐ?¢ÐAï‹)OTHER4FGL J1910.7-5320¿Õwoå¸xyÀ8>A_EàµÀ:~ùc<À<b
@@M…XÄè'@$$D'æÐ?Å6w
x~í?ُã¢Ò'€@•›Þwì?øöûú·Á£¿è›n»Ÿ}ß¿Å£œQÚ¾¿ä6žÂÎFJ¿çGú D®†¿îÒWPHí°?Ҕ«]¼HÆUNASNone3FGL J1911.1-5318?åh£ì?#?Ã
S>O'?Ê ¨þ!À?Àùӏ£ed?ÀBO¦´?±³Éñé q?梀'œk?Æðø¿Þ—?É|5ª½y?ÂÃԑÎZR?·ó *44?°‡}š¸?áöá1ÍqQ?´/L…Õò"?΅q0;S‹?±¶¨qno?ɟ
Žç0?«‹|Õ¦€¬?âMµ«{¡ê?«I££±×?Ñl†!í'?¨b§ƒÖÓ{?Ãï¤C§Û¸?¥Äë—h;ÿ?Þîó³k|Ñ?Ź¾:bÒ?Ó£R¦§/k?Å:0Iì)¬?ÊÛsKÚ§‰?»%¦¾×Qò?Ùoâ›Á-?̪J–Ò	?Ûº2àkÔÔ?ÍìKÒ?Å«Õ	Ëõ{?º¼©Ôz@8?ÚÀî."³ž?·zÝ2Hó&?ՋBÚ¬D¨?¸ïK¥5}<?Ïgí€t?±Ám¹"R?Ê'ùKäbž?§Z!Œ&Eb?àɱÙù¨o?¸Œëqü½B?ÑXŸ¦}Ò?¶F,×îMIXED4FGL J1910.8+6300?ì^œ‹;ˆ@5Ø6¸ù±1À;eszK¹À<åyéÐé'@ .e2§?ÿ`UÆ2o?ÌC">™BÝ?ö©à8º\?ôˆ²ÁˆÌ@{2ü+µ?í‰?MóÔ¿ï韛†&?ïÄ÷u³¿åÎéõÒ¿ÖÍY$3ü¿ïÿÕ7ÕYcUNASNone?JÚÍ?"­QÞú3Ô?[ÐҎ­UW?VñÈ«?"äc"ä~
?'Ø*-=?ï¹@²'|?Û4U/yñ?U´J`P—?aOÝsp3?~ù'¥?~9.qpó?îލk§³?""!Ê%À?^H—&Gî?c­xçÑï¤?¡-rš(?"iNoœ?ï¯5q?Í?g¨÷cÛèæ?Ok(%w?CýµßÅ£?';ê»~?f3"ƒÜ?ï‰rô®?˜7p2™?k´"7b\?ert °??›˜?&†|†?–Ép»˜¶´?ïQ\òÒÎ?–öÛ¦/‹?c&r1Uˆ?seœ'Ó<§?"yFw±H?"‡nå4#}?í'7=ëU?£¤¤;hsÍ?fáùf,-?kÍ×ԇÀ?³76Dú?£"¬pI?ï!µŠ'Ù?‡ŽŽ$zƋ?_œŒòýó?]~6‹06?™Ù2¬g¶ú?†ÛœvØIdAGN4FGL J1911.1-3221?ÛS΃ÜÀ1ùÊâ°À:À1"öÂjÀ<BWڎV@í§¸Á'@Ñ>Eþ?ÑZ¨VÌ?Ԁo|Ä>@H÷}z"@ÙÙ7"@ê?é÷•ÞN)"?ãâ`b@fø¿àî`/뀿áñĞ*"¿îŸg~¿M³¿ïý"€U$öUNASNone?îŽù)n…¼?"¡Ûð.?ƒ¹
Œ_fC?v³[\|?¢"*z13?'¦{
ï*?ïJ°…. ?'9¤t:¥È?yÖ¸Ý{?ªõë^È4?4w¯E›?‰ùž¾¦×?î?þÊ9¹N?—ó[uÕ@Ð?"äM"ñ½?‹â¡³4?¡õ¡9BŽ<?lêí|Î:?í+p×-£Ò?‡ÍSiæKð?›ÄÁh²?xc9ÅMnt?¯¼.N܂?'ûIÝ¥ªM?íK#ÍÃ?¡ŽT7¬íô?–а·6pQ?Š•t¤uH_?¯åjÊƄ¬?œ"$;qæº?î›´ô5i?¨Óxg¹°b?"$¡Ä"÷?šxâÁ‹
*?¥óõÝFªz?¢«Ó³î?ì¡q::?£·âXDýš?¢tõqòæ±?"æ!©ëBÑ?±¹ü¾~–¹?"êöÐÏ?ê\ƒc¢?Ÿ»âi£$
?§fR߬±?X/î}'?ÁÚޟL?›têÄ¢AGN4FGL J1911.3+1055?ã#P°­Ãƒ?ãgpQ¡³À99ˆ{¯¤À:•¦†è½@¡'Œ_t@íŒ_õ3?ÚBj?ÒËÊCZ°@r=äg?ú=k€3í¿ïõ¥¾Àðv?ïÿŽñ ¿çHÌAâx†¿çË,^WÏ¿í8="ßEu¿ïüÙçUNASNone?Ýâ\sìî?Ç9 …E?ÐéÎí°¿r?ÆY»õ±iç?Ñ3ԟ:SŸ?Äx}·ˆ9l?¯f‰ÌÇïB?±å2çÏUÀ?—w5@©"?ºÂŒ¤1M?éc¹•ãV§?¾»ßÌ{:«?Ê,~@Ö=?­õfð‹)%?ʐâ濒'?°úy]ƒ?âÛ¼&¿åç?³ç;G…¤?¹#ɑøÉ?"+š×LÒ?Èuð?©Oà¨v×"?æÕ]©m;?©ÙŒL~Ö?Ó¼€;+w?Á®ÝTAS?ØCx|àÈ¥?ÊXªÕÅދ?ÔHä?ÆÞOõp~?¡ØS#ú—G?¥x
3ÒÃÆ?Í¡e"¶3a?Ç5ŠyHÉÑ?çz!hÒɳ?Ǜ#Ì&Îe?À*•J)™×?¤P¢iRÓ,?ÐWpã¨?¶3ړƒ?ãÉ¢;åÅ}?¶¼%˜ÕtG? bëS<ìY?†âC)ëùÈ?Æâ¥Å)ç?·°(÷!'?éA'ÙtQ?·Ké§V¤MIXED4FGL J1911.4-4856¿íÄ\¯i ¿À7B«%(®À;5Ÿ>HÀÀ<óK¯Ri@vǕ«Mv?ÿ-gwžZ?Ðþ!ÃõÝ?èIè^9q@àýÜ9Q@ÊÇU> Ð?™cÿÙ¿y}? N>§?ÄHôe˜
M¿åÂ2᱿ïÿ;2G?߉ˆ>þB'UNASNone?ãN
¢ˆ‰/?Æßœbˆ?Óáò×VH?ÄjmˆO?¶ǎcIj?¬Ûnmta?åŸRò~?Ç-‡Í"Gö?̏y(ϛÎ?îd»Û&Ç?¹æ}fÌ×x?°Í=×n>â?áÒ_ÚÏç?µË´ x?Ó. ÿ`ë?³Pf~?ÂYA­Òê&?§NÊ¬ÄÁ?éH¼•ó?¤9A4?Âî/YE&â?¢¸g¹Bnt?±)`Àlé¤?'U}¾zW=?Ýw¤.üu?ÆrÓZ§ä?Ûj'BE?ÆVD²Dû?¾"ò:?´¬ÕCeq?Þm
'}%ù?̇¾ºÌ€?Ö­ûÀJ?ÌTÆùªô?ÅÉîöî3z?¼§ÒàjÁó?Ù²ãf0$z?¸‹÷#ˆQe?Úá[nO®?¹AfEOª?Æ׃ñ?­C§œ'»?áæòveÉ?³ÌªÿLŹ?ÑçqßnÌ?´¯çÖãë?ĕT©þ?§J`b œMIXED4FGL J1911.8+1447¿Ò[ôÀå@•@?ºÆà$À:-±4ÀÑíÀ;{miç@!A×0}÷'@˜¤§Ö?Âå9?¼®r¿—}4E?ÔïäÿÉy[@æÊ6Åcø?äE~Åý0¿á®å%‰&…¿çÅàŸgŽÚ¿è–•Ù¹¿¥¢¿76¿â›`^©UNASNone?Üûª–2?ÃņԽS?n¯h¡Ëµ?aˆ*Ìé?ác{‰}©?Ã([¼œÜx?àÕÌUñ?Í,ß&k¤"?"RµjÁ¦?šð¨–"Ù?Ý<š©Ó½?̞¹(«õ?âÛöLRp?²èê¾ô?'{ºéþê_?…õqk.™?Ù0W¹ØÜÙ?²Ûýˆ|G?ç°ÃdCK"?¦xŠi¸Í?qã24õ›ô?`ÄQ°L:£?ÐVìn[Zø?¦‹‹ðÖÅ´?Ò†S|åë?Á‰þ›üË?©‡"s\?uø‹Úx¸Í?æ¿éÈcº?Á\³ÌÃ	!?ÒNy$¯ò?Ƶ'Øy2?'€…6æ? ög¾¿¾¨?æOÓbCÏ?Lj֎þœ?ÖK#ÿ'¾?³ª—)€A?¢ˆ"aŸoV?—¶Æn?ã±ëÚ{ƒ{?´9ytäú?Ú#'x˜÷?³µ6îì–É?"ò%'Yàü?u/kKR7?âšn­ÕP?´E›.ˆîMIXED4FGL J1912.0+0927?î°7ÒnC¿Ìæ'Ú]"À8ÓbÀ:ÉîËû@Ÿ¼wjÏ@£ß¾AÏ?Ëṳ́ÞÇ ?Ô~ÊuÚw°@DG!ý€Ê?õiҩۆ#?ÑώH,¿|¿æ…¦2.Pu¿â¿-§Ù¿æÛWãä¿ïi§Šóä¿éb`¢­ŸUNASNone?§âVh?Ð?­C'GH?˜‰ª @
‰?•Ó	-ÏfÈ?í½HlD;?°S²‹;"?³žš_Õ70?µ!-S?À$Ò>ç5?´ŒIqZ'¥?é'ø0¹í]?¸¨X/Ì3e?¹)'­µS‹?¤¯Àˆ3?ÃWüùÞä?¬m§Ãëâ?èÐl>—•?°Þª¡‰?†¹ ÞÌóq?kòiØ"6?¹}·%ޛ]?š&CÈFë?ìud—ÈøÇ?›^¼§O_›?¦<ta ?—ˆ³øɊ?šj'Òr–?—LåfÀ?î§z-b?¢aЗ—Ó?›ZÚ=¹ú?¡¤‰ñ1»L?úU¢…Ô?½0¡'j?ê6"Åš(‹?¼f´¦ ¡Ç?°'XOöƒ?˜¤Â¿3q?ÂI°å²ï#?­V$ ‡?éh¨¼]z?°8ósê-?e¤ØÀ·œå?S~)u$/?¼Õowuò?£i" P?ìO­80Š?£Š~r3ÀOTHER4FGL J1912.2-3636?àƒƒæ‡'À3­Hˆ/À9û‰ø;æ`À;n'å".(@t9)ÂF6@§%?Tª?Ð^?ÜV?ϑ+6¯Æ@ëÅÃď@þü—À¦y?îÚ)'z¿ÕLÉè=ì¿éô§<‹Â¿éœhKBôq¿ëò`°
¿ÑŒ'Á)iUNASNone?îÒ6Iàk?—Ê㈬á?}1Ôµ$–?tÒË~Œ¯?žpÖCþcq?•Ûx6G·?îT!¹Òã×?«´ÜZÓC?–àÜò7?Ÿò!¬3`?ž›)Š'ë?¢ðÙ¥À?èo`!Ë#L?­H°X˜"?¢Ç»v%Z´?"Õ
#""·?ɐ›ï	c?«¥`÷6ŽÐ?å|Ð6Iú0?¡Šç›¾ã?±[Rºv¯?Šƒ{žQ§L?пȿ™Tó? ¯»d$N?ì]/2ßô?±œë[´{?¢€[[О?XûJÙ?´CPM$•?­R I¦±?êI~ño?Ä'x/ø§W?¹ŸÍ"Œ®>?¾é7Ͳáû?¶æqÂÆ?³Ñ5@˜eV?âIï˜v%?²¶føRN¼?²®I0Îé'? a§$q¤]?ÖÂEÔd_•?±Â©Íu<Ž?Ôbg"ùÕ?¦<ä{®æÍ?ÁílÎúo?¦;Ð~~'?áSq:ĐØ?­˜Þº‰IMIXED4FGL J1912.2+3621?Ö%Ç|xBÿ@'¬ì O*àÀ;˜Ø?ǖ,À<Ôe›eK´@(p¬@» ÒÞ_?Ü!3 ¾¼i?îbÑ¡GãÄ@
qU'Ù‹ø?þ:ñbÙ>?îAŸÝ€y¿ÓáP|ð§¿ÌËD˜¿ì·c^t)ž¿ïÿÞý¦ßR¿ï÷@s–VUNASNone?è%Âýô•œ?Á´f=e€?«ê_g–'¤?¥'È|ö?Èn\-l8§?¿
|ªËp+?à.óÂsÇ<?Ñ~"ºåC¼?ҙ`Tº¨™?̼R8(‡Ö?ÊpL»'Þ?Ȁèƒó¦?è‰ïÑoÚë?®8¶d\t@?»4K®v˜?¤IäeõÇ%?ÀL&"iY
?¥
[>hf?Ûg>üGÂ??°a{5?Üa
dRÌ?°ž™+T]?ÀoYì§Õê?¥FËÖؔV?á'â÷—·Ó?ÄÎ-Í4H?ÀÁ–‰2?³õ÷O˜ž¼?ÔÎÙEÅËÀ?Ä^Õ<KÏ?Ñu%<`¿š?ϊç;ÛD×?ÝÍøoט?Ñ肥·44?мâSǨK?ǔ_}¾òš?åÐY?³*L(Œä?Ä[¦2Èîá?®,Ùf‰?Ç`&ŒÂ×½?ª±gD‰?ÅǧûBg??«R"ȁW'?âóÌI*|'?¾..D>¦â?Îi&à¦{?¹µ•¬,ÌÅMIXED4FGL J1912.5+1320¿ïì²%+³?÷*ՖŸêÀ90‹µ«HÀ:ºðY|s@Ý$zØç@
¸·a+?ÇÅÿ©?ÔæÈ •¡½@àÆÜÈÃS?ýݹ\~0?é"Ë ¥<¿âõ:ªù›¿ç)ë‹Ô´ù¿ê^æ?d™Þ¿ïø~eET¿ïзþ^•7UNASNone?¼5<s‰ö ?´¾3<¼uœ?¹˜"ƒà
F?±ò^}z?éFT!.<Ã?¿¦¨˜1‡?Ç®ˆËk+?ÅW{(·¦—?ÄdZ²þð`?¹9ÌÀ½"Ø?äûGLMi?ÅÝ°ÄG[ù?Ð9Eç÷‰?°†$ï§?Àß»zG¢_?§T‡Ú?ã«n-㛤?²ï0	ڋ?µNcà+!·?'µÿ»´?Ãi¿ÊŽa¶?›wŐ@Ë?è{Ñ©yû?¢Œ{éyc–?¶2Žo/h?­Ñ\ÌÙ?´¤	Œ«%†?­røqˇ?ê¨|Åð²?¸KG"çÆ?°–à›è|¡?·3±*¬gW?Ħcûì¹Á?¿ÓÑýýá?èÊ핀l?ÂèPÁŽ€6?Âb"™¶† ?¥Ð®ŒM‰S?¿†d{³2P?§‡ß8Þc?çvŽŠø.?°éAbûí?—0qÚ/XU?|Géß5w?ƚ¥¤%?¦b5—K ?éŸÓà…M?§ª¦áoŠìOTHER4FGL J1912.7+4610¿Éë1¶JC4@/rÿÑÜ×À:Ï7Žâ†rÀ<¤¦Æ¨Æ]@W˜·Š @¬À½ÊÑ?Ŭï¢9Ñ2?×
;|Øæ@®0‡‡H^@0X,¼Ìz¿ÑŒž
²?ïcìÊì"¿á­˜‰Ï!;¿à—Lg"t¿ë!á1ßÈ¿ïÿý¡UûŠUNASNone3FGL J1912.7+4610?æo0ôáá(?ÀJUP`âæ?ÍèQk55Ê?¾­vßõv?°µÕª¤)?¢<·$ƾ?ës‹Y~»6?»‹«"
Êg?³&‡‡'?²>ËodÖ?°â~­u'«?¬zºÑ²?å"C¾	ª=?´&2\³/#?ÌxrÂë!¢?±y}BS•1?ºtü…çÞ?£Hh?ë«y‡eK?'61
•Ê?¶<4
_»?Ž£‡PŽ/P?¨ÏÿÒË£ß?ØOƒìO?äs.b‹\â?Áےœi'?Ñ==™yÊX?Á?e'ù9?·q–"!'?ª9‡aé?æ+K›'uÂ?Ä>£¶ \ú?ÅÜçŸêt0?ÀÉ<ßÚE±?ÁuéñË´Ê?´¨°Zµµ?à_mÓË¢?¸›ño"àp?Õcy+åáò?¸´òQ]ï?ü»ó
Ï?«&^æú§O?æ £˜ÃRG?¦õ°´§â¿?ÈäÒó~?¥%Fsraž?½2·'–Ò?–w}@2ûAGN4FGL J1912.7+0957?ï1Ð]ô¿Â¡«`ìSüÀ8™‰!|QŠÀ9ÿ¦sœ¯Ï@>Ž2Þ#·@æÕw–?É;΢ºÕ~?×B-'ð
@~Ò`Š"S@Œ1>fm¿îô‡%ùŽÍ?ïÐý¤-¿åȪ(]\¿çò—a°õ¿ïrÂ)ۛ?±	5ô–UNASNone?²Ü :¯?´sÔ½t$?£Ç%óùo??£¡¡çÿ€?ì)Å: &?·°]ÍDÿª?¸€Ê4;ýÏ?¸þ`o`É?Î@ÿäýG?À¶šâR4?å_¦¿Ù¥?Á±ÏZñ"+?ÁL['Òû?®@9÷Š ?ÃG‰ªÃ–?«;Gí"}?æÛÓÑ\?³C9g_?žZC¸ÿtò?'9Â&ª1?óÉR'>Ï?¢+ŽIël±?ê ;…ö5?£m­"²¶?—ö? ¢?±›šS=?§Æ^½ˆ]È?¦gj¢)?íÃèK¤³?­Gúy/ <?ž©Õs[ä¥?¤©t¯´ ø?ÔA½å~J?ǒڴR=Ì?åu·æ?ÆñüÅk?·8Ó̔o?£er…¯…?ÄâϲI?®ËÂ¥pV?èSìÄÂp?±Á®Åu?~ÿwÇEO?j·ÈÐ\-?ÇÅ|ÃÂYy?­uîýJÚI?éСßt€l?­Ýq­
â
OTHER4FGL J1913.4-1526¿ëL"åB‡À'}ÚH¶R7À:¤$'–GÖÀ<ƒ¶85Ñs@¤¬é¶¹?ý+oðS?Ïd'œÒK?æðbžZÉz@‹&|k‹i@)WÅ8Ù»?ïéϘY(?ÒÝ¢] w¿»4J	Žt"¿àçÏAǺ¿ïùŒž^z_¿îTœÚ–¹ëUNASNone?׊Æ©?ŀîgóž?ߢœ9S€'?Æ#qZqvÌ?Á¦ÄÅx?·S_øÎ?ËÕ4ËõȀ?Äᆓ钑?á}R¥G?ǯ7M²C?Î6Éév.c?Ãõ:>À/0?ÓK‡vñê?²€	ß(¤L?álÿVÚ#Å?´ñän?ôó¶µM?§ÉSv˜ºV?ÚßdfSh?¨n'¶©ÓV?ØØ®«R¡?­åáoìØù?ȏÛ,‰¿? œþ­²?ÐhÆ֜7?ÀŒlŠlÕì?âÒ||R`ö?Ä\'ÓsýJ?Ãä€a~?º'×׺3?ƒn<§.?Á~ú‹Ø?㵬jŠ@?Ìk
õ¶ûÕ?ÏÊçšX†?ÈuPç£<?Ƃѽ2·?®Mͦ,A?å:¤Îxjí?µe¦˜ª§?Ē›ë.?«©}vÕÈ?ʙa ½uþ?§þ²ŠÔ?ßÖJ±Ìb¼?·¿¼ÏØ?ÒݽÔâE?±>LëulMIXED4FGL J1913.4-2652¿Ô7½lóÛÀ0c÷œ"/¥À:ºØ´5&À<cAfҜð@ž«¼±Ì–@œ':×lc?ÖiÀãàd¯?ïГ*êU@؍]b²?öô¾
'*:?ïîj}L¿Ö´¯àÄ¿ê†Jg,_¿ïõþ~pH¿èup¾®ý¿ï‰:;e0ÜUNASNone?éW(ª\ú?ÄGx5yg?ŸÈ÷Öì‡?¬°ü}7ºâ?ƪ>[Ê?Â{ÆIûÍ?âdjŒ!A?Òûw…´í?ՉϳBH?ÑI
$«°ó?¸n"_N-Û?¶ƒÄÄ`?äÆ	%\tº?²á+ÀNï?Âkh®Àe?©â°b(¬+?Ê|r½óÒ0?¯Ww!~è¯?Í8bè,¤¤?¬ÙlF¾ð?ã"`
gô?´xMivXz?Ävî3‹?¤lÒ¬\U?æˆùŘ÷?Ç1÷²1H«?£ÌQI@?£GZá_?Ѝ	;E®é?ÅîЇ\$?Ôâëç3L?ҏ#9ý
?áj½ ßÞø?Óَâ¹ý?À1°@?¼xhò\ÔA?ádž]?µkLê"]ð?É¢'
-\|?°—QÎ
p?Ðe'دP‡?²V'ÉBŠ±?¯6f0›?œ3"úÓ[·?獀wb?º‡~'çêN?Êð‰À]©?µÂUgŸþ6MIXED4FGL J1913.5-0923¿Ò÷tøò¼îÀ"FQ	¿À:?þ@_ŠÀ;œò™åï´@OcJµ†@fnŽ›9?Æù¬¿;>Å?¡ç®ƒMî?Û⍩K@ϒ¾^¿Ð¸W_bf'¿æ ñ—‡q¿ìðŽ]{[@¿ÛÓ&Á½¥¿ë[Ë}lg\¿£f_Î@UNASNone?áüò˜R?Çbrw'?|¨s.à?qï9y+7?ە,†ŠŒû?Çú{·˜?ê>/ªV?¾°g¯oLr?qñêŽÑ?x‡uv`?Çg«w‰ñ¨?¾e‰i=?è¡0ŠÈ ?¯ý².?–r˜ÙF?Ž"l¼k֓?ʧùÐø?®´†™‡‡?î'Í, ÍÞ?‰YŽ}†?hR¾£õ)?KFLµy?Ð?¬ø
ÿXL?ˆžÂg2 ?Õð˜a"Ì?ÅÞkûѝ?ë,=³…L?‰µ3b‰á5?äýÛx2õ?Æ Á'BH‹?ãg»'+ªí?ÈZ—2-œ?u"$Ê].v?ïÆEú?ØÚxH³o{?È<3y¡y?âHhKîÀè?²ï±KŽŠ!?¥¶D_|¥?–Hmyw‡˜?ظfä:§œ?²""Fj*h?ê…ýóË?¥HÐbàHJ?'û¾
?lѨNÆû?ĸP^ZB?¤âý%~ÅMIXED4FGL J1914.6-1157?î.ÀK£Ü,À%È%žÀ:Ë©·À;'gÞ5ªÝ@¼3ù¬©Â@ðRãÒ¢Ð?Ì)³ʅu?Öﺢþ)@Oá|‡:?ÿՐx2Áž?ï±åàïïg¿æYôhI¿â­[þX‹¿ëA«"ªO¿ð?ïû÷"IôUNASNone?ۆ¨ð="	?ÆC5…"?§¿¶ê?¦Û
½ŽÞƒ?àÀ°&xåš?Æ6â+]?äƒV—øjñ?Èàë°Æ9"?«'fՃ?°ùŸtÂ"9?Ӈ%õCI½?Æuó«?ߟAsè°?³!ŽsŠ?µdU'þ?Ÿ>ëœG~,?Û©+ ÙÙ?²ÄoÃø¶â?‽Ž&¯þ?¯.¬Ý`?³ ΍´?'?^ƒ¦º«?Ö8ÿZ¾'w?¬Cör4;K?Ö}­¶˜>6?NJpgÅ?°™8ø?¯ŠÆIÔI?â½VC†"?DZjµoQá?×1¥ÈÃ?ÌqkÊv?Â;UÒ«š3?ÃTwæì]·?ßÛ#pâ/#?Í™+yo?Ô§{\Ë:¯?²RpG2;?¸Ò1D(u€?£Uôºc?â'ü)0ÐØ?³û"þð¯'?ÏõÑÄ¿sY?®‡Ye¡ðU?¿2×OªÁ?¤=Æ_u;?ä0¤Úâ²?°ò–ŸüûMIXED4FGL J1914.7+1012c?èÕ×z¥¸Œ¿Ý3qÜç!7À8ÎFèòAÀ:6Ô­kÞu@OîýNIå@•ÁF†Í?ˬâa3¡˜?Ð+ØËސD@	]5<ø®Ó?â8èDU"$¿æ»/€÷e?ïõ8áÈÝT¿èÛª¶!¿æš¶š[`y¿æÄI,«¿ï—ªÝŽ¼UNASNone8?½D•Æ¦B?ÀŒíÛ ‰?¢ACxB?¨-§ç8?ë7m3Mùø?Á̲FŽ°?¹,)ÒÈ?º¨jJ3?Ç®ò`¨?¾®yÖ]?æî¾D|d]?ÀûÞæ³[?¹‰¥"PcÙ?¤`úë?È>ðÃCƒ…?±€oßE|4?æ¿Üc?³-k[vPó?'úç­ÇЙ?uå=næá£?Ç@˜ «?§$³DŽÅî?é˜Ü2ÆQ?¨Ðc~V?µW'Tím?ºu\õv? ~ŸÝÊXÑ?¥Ó]:¼Á?ìM#·j:?½8ܼ6°?žúF½%?£ÙØNæ6
?ÎCŠ¡â›õ?ŬHÈÆ­Ï?ç~½ƒ6^i?Åó»µ4?´Î'¾-øŒ?ž'+?© ;?ȳîô-Ӓ?³«Ú1?ç92s":?³í\QS?wuð2ß?d'²©cÓ?ÊI¯mã«?°–(5~<?éJ³Éƈ?°Â¥xbOTHER4FGL J1916.8-3025?ÔÝaÆ&À2k‡	VÁÀ9ÀUWJi±À<2š†ÿ@ך¤["{?ü¡m¾I|K?¼((¾DÁ?Ñ|vžÏ@pÛjË?ùt(ì]`ٿ䇱°¿ã­¥àNß·¿Êf€Ä`˜¿Ü;Bö…¿êþþ"ZGõ¿æã"GþqUNASNone3FGL J1917.1-3024?å»<á?ÁnÄE2~?Й%¹Uª4?ÀA~ê/£?¯ƒK¬)S?¢$
¨þÐü?âá'R)m?È[Ó)Lv?ӑ\X?Ɗúuã˜'?º²nùC3˜?²9MâÚ?ß;¨-—N!?¶䀡Ô?Ø0ƒ
aø?µQ¤ÄbH‰?Á'©_Í?§C$êÂ?âÎÔÎ<Ó4?¤ÖJ{ò?Ádâ,ÛUQ?™Ý ÈpžX?ѯåLÎ1?£‰Á¤‰ä?Ô:Ž3Ï?Á! Ócƒ¢?áËÑáDå?Ãí`¸sò?À[œëkì?°é£EŠ'?Õ7Lh?É2™_?´?à¶0u£ˆ?Ì¢òÀž¸Š?¹"Ç??¹³ÔòúÍ«?Òû–@k!ƒ?¶Ù')þ?ázKÿž?¹ê#Æiík?ÄêO-~'?©°¥×mú)?×:ó­"q?«|ËÛõ¯?ÈZ3	91?ªhÎsª;?ܗòÏY³¿?°£ý¼•lMIXED4FGL J1917.6+2609¿ëBÎeܱ@BèbTˆîÀ:\p\‰mÒÀ;ű܆~4@šš"P1F@§Jº8u'?ÅmbÁ_?œš±,ç?ÊL齞\?ñ'ç[ne¹?ïþ.H‰Ý¿æ»áWžL‡¿ëÄþÍ%¿èÄ$½Nªˆ¿ÒZaueݪ¿Û3Üȃ<UNASNone?ÞQµ`/Ñ»?Ì&ê½²?'qQE©Ã?¯îIéö?àŠgç4?Ì-èèٕ*?ååSΫ—?èO…àel?˜[|"Ô|§?›µjjÒ?ÔJ}ŽîgI?ÂOÙSBO?ç‹
?'?¯¹"±Žˆ
?›ç$¯aB?Ñâ¶CŒ?ÎVå)ñO?®Á¾	Í?ëKóã*÷? Û7þÜÚÛ?†<fB8?qEL&Õoô?	ÊÑlf? +xÍ8†?ÕôÚÆæs?dž¬¯|–?‹2
'ÿ"?'Ò­…‹z?ä˜ÊÍÕFª?ÇÂj¾'?Ø=9oý?Å0ü2|:I?¢¦_ò FÜ?ªìw®ˆ5?â·
d>¡?Ä1y'ÆŸ??áŽ'Jj²?´n_á­~?¦²üH
Öo?–oà±²ÊU?Ú
ŸT2v?´‹U¼¨šò?ãÍ­\?³©E^k?b"‹/4?…
à,>ç?Ø(;lwS?³P+ÕZŠÇMIXED4FGL J1917.6-3204?îY}ÔZúfÀ3*0"ÝzšÀ:CbzH›zÀ<*.y@-·qEèm@v"aKts?ÈS7_'·¨?о‰]aZ
@X/ž‹q?ý²-V?ï¹#!ÃM¿å]ñLÞÕä¿Þæg}'§ã¿çh¼LLí¿ê–`ÿõE¿ïÿ™s,ÛUNASNone?íÎ-€Òßr?¡"-?s6?†'9(Àj?{ľ=laó?­xÙ©«¿Ê?Ÿ<KhfÏK?î]]kd? íyæ=ß?"åãË	Ê?•Òpzg?ŸvñXZO¦?•ÝûsS^Í?ì=b?Ôð÷?£^WÛ%ƒ‡?¢""T¾ÑÀ?•yf¹Áƒù?´Ê£ØBéã?ž+ÇÞ[è?ê¡®Êi_?"Kàôº0?«"²¯*«?ƒrQ¤c£?½)Õð®?Žý‹}ïfw?éÀߤ¬ó?¶X-pÂ? A|"yI?"âòí·—Ë?Äì$‡Z
#?´PêSEw?ë5œÏ®ÿ\?·V$
¡4`?°»Çƒòa?°Äéٖíi?µ—Qýº½?®YJ%Ç?è®[¢_ˆH?®q?I¡F¨?±›3Z	M? cȳTÚ?Äx÷Ǒ{?¨a0á8-ˆ?äÖ<Ö'Çù?¤ÛÁüN?¹"´BáS?˜üe¹Ì?Ðáf":Ú?¢BÀJ4AGN4FGL J1918.6-7813c¿ÛÆ7ÈÕWœÀ;æ·ª%ÙÀ:yl2š‡À<$aX"@ѧ*{ԍ@±ƒÞFqÔ?Ó@¼Þ˜&R?׈^2æ1?ûßFfìž#@Œ G2Ä?ï¾
'*:¿ÓíIå&_æ¿é´â_ܪ¿îú´|lb?з,<f¿ï¥c¯˜	UNASNone3FGL J1925.8-7826$?ï,@nôÄ&?–þ;		vÉ?hP¹lLù;?hjýlÚKI?—mÚô¹Ã?•RGºB R?ïVüé†R?•"y"µl?s›7%?€_|öIj§?Gy_i&r?ŽC}
ö0Ò?í
…´+ã€? ¤» R?šØ4¢¥ ?'eá‹i¸Ó?°ÝÅ6 :˜?šr	'õ?ï×û÷T,?'û¥z'á ?W.øÏ&ɹ?N‰5ÁΧF?œ'îw²ã?'a*æ?î\bÆ7¡?¥'#ü¤úÍ?|¼"¨¾"›?uyßT
Ý?¦¢A,%??£]t õ?îcEЀ?²º˜}j?‡"㱨Ÿ•?˜´¤«Ô+Q?©d–¬¥?®Ø¤Î)cê?êm"è.Êe?©!loì[?«À$oag?œÕN,‡F?¿ˆ®å±?£s¯WÏ}_?ìòÀf¯Y?¢V¶†i…
?pPáè'y?mƒn"20?·jëß3B'?¡Ùz?úAGN4FGL J1919.4+1313¿çd¡w´l"¿µàK¯«ÕÀ8YÂÅ+À9úád3†?@ïf£M!œ@w$ÄÛfÄ?Èڌ(õe?ÞUœŸ]}ß@žK¢•Áž?ÿQünûá7?ïï>ÜÇ?® ÃDõ1¿è'âôV¿íœáL¶'ø¿ïÿ¥!b%d?ïøDRëUNASNone?ò`ãx>?Ãe?¦D^?§£u
'²?±,sÞ@Š?é™C×VyÅ?ÅÇ÷)9?Â^—7ó?Á¼|XQ?ÉÍ´€r"ª?¿P%¥^§^?äôíæ²Q?Ä:qu¹´?ÌR®‰Ñâ?±õÞ8'?Ã.›Á3ˆæ?¬IM´VT?ä/Dd©N?µ°h\)ê?˜Ù£f?'vf+]œØ?Æ]¼¢)­?¨Wš1Ó.?é¡í£å€€?ªÐø²M?°Ÿ&‰µ(Ÿ?ºüÌ7Tý?°7ì0©¤?¶bìIVð"?ëå­~˜?Ã3Ï:eW?¤ì[³Z

?¯âݬÚC?ͯ4ݦ\?āÖüí3?çEm
…µÈ?Åès»}?Å`³ÖÔ?®¶B¿Á?´%Á°Žÿ?®´Y¾=T?åúəÞÛ:?¶&2Ó«§þ?sÖ´ìT&F?bÛסýïA?ËÊU}yÂ(?´¶'¼,Vû?èå½6àD?´òý§Ï×OTHER4FGL J1920.0-2622?åç}€ðf–À1"ÙºÀ:MV¿)vÀ<V'Tà@.ô®¾@I}<kÁ?Ç׫£Ì?Ò¡ä@Ü¿@
ª"Àā@4æv"1?ð?Ð'UØy©¿ãŽO¹{·¿åÀÌäIÁ¿ìˆ[NoÑ¿Ñ&w ÈÍUNASNone?ì;蕨?¶¢´m>ùŽ? ".};Ëû?˜ÞyÛSÇT?¶¨´Ù ?´O̤'wë?í§ZU&¨?ªìÑ'?¢¨$¦/? ÞþýŒ¸?¢â6‹?TM? =×ÔwAÿ?éfÕ07o?­ÿ£F"?°pòÈ&M[?ø>=óï?Â,1َH¥?§àTmYc?éæ"}dÒ?•^yR¿?µä_'¯?Œ­eÛ$t?ºç?@Ö?'W:û"/?æÊÏ$H'I?ÀÍݽy·k?¸Ä¬¾ã ¼?±")zC?Èrm¢à??¼*›äÒc?é×[—ª?ÁÉðjqôö?¿ž¿!­=ª?»A•?y=?·ê†߇?²lWaeˌ?äôG·=ˆ;?²óÐö¹?¾ß~{íŠ?¥žŠ+Rï/?Ì¿!åPÑ?­´'7Èw?áfú/±s€?¤êÌþP"?Êu=;AA?¤ñ'8å?Ð1Ñ엡?¥
Ä9ŒZðAGN4FGL J1920.7+1334¿×qAJ;ý ¿È‰S¦EN"À9Êc&3À;vރ®uÊ@/ Ô ~%@Á›@bƟ?×ÓDç:·?ï•ÆÁ#@9Ë@D†r'&?ì®rn²e¿îZièÑæ?ÀË(²Ñ¤¿ê€ïHø—V¿ï÷Ú,0às¿ïÿüÉï£UNASNone?½N£ÀÓ´?¶_3õ@'~?¶·úœ'œ?¯"¯»¬?é–ˆ'ù+?½Ý¤"ü)d?­:4çåÃC?³h öÑ?È¥­C?ÁьQSüú?è&ׇ澻?Á؝&J?Ñ2{Ýñã2?¯Žúž(?Å8x9?©Bíó/"t?â!€ËÂ`¸?²˜Râ³»?¸Û"W"a?š'"GøÙ?ÛÚC™nÝ?µþ-Hž»?ÝîÛP¯V+?µmÈõ°?£ƒ})t¹(?¢:gLBãO?´'…z³x?±‰÷ƒ?ì5—~-Ͼ?¶ŒG?ø?š"´I'?¡p_•e"1?Åø5ï6?Ã)rȨœ?é»·;Ñ?tZüÖ?Áõã*¡2?¦ üğ_?Å©¤zYs ?­k®ß?æÁb‹?²J&VE:?™=%×(f?‡$˜÷ÄXp?ÝczIƒgå?À?šÎçø?à"Y¬wJm?ÀÙ=Z»OTHER4FGL J1922.4+1453c?ê¹æó…Z?­ºãôº/À8ɼHKÀ:%ç}R@ó¨9Dš9@©K£l3?ÐTa¡Z®!?ÚAœ¬s'@‰¤Òh@
‰ºr¿íxÚÂXՄ¿™¼S`'Õ;¿çJè3FS¿êÙ๨¿îª,ŽÔD¿ðUNASNone8?¿o˜?ÉûÑ«Xß? m@=enÍ?¨õ€…'}¢?êIP~ê?ʃ§–:?·ò‹üŒ©?¶¥xˆÈ~?½anÒ=Œ?²›&K¡È?é`ÔN?»+»Û
p?¸4"Iˏ?¤§ÙâÛ?ÀQXÀ¿?¦ý JÏçF?èåFm¢›?¯K‰°âCS?¡–Ýù+5Ê?"¢Û…ö€?¶ž‡ 4ø·?—Ç/¾–…?ìÁ,tkü?œ°%9Yï´?´P;FØ?Ë7ßÀD~4?¡lçÒ@‹?¤rv9Gh?ì_*ÙðÍ?ÊݖɅš‰?¢9×+êLa?¤iŽâL	?ÃÖg
%Gã?½Ž3ì¸òÈ?éæÈÊÅDZ?¾ œ?±!2´ðþ~?›Ì¿ñ#¦?Á¹ÿuk'ô?«Š^ì‰&?émYË´…?¯ƒuÃ`?' r>Gvª?n×5).Z?¹Ï™tŸ}ù?¡ÝxBf>ê?ì{‹(º×?¢näb‹R"OTHER4FGL J1922.5-5233?é"'.ÃÀ9͋¤
âÀ:w¢'^<À<tñ´âg@ ÖQ…Ú@M œÃ?Ç6E¡ÊÀƒ?Ñ2%acr@@™'6@3{ùö{?îú÷íâÇ
¿Ê$ï"¸Ó¿áæüŽ[wö¿éC>n$Ì¿ét(%¸÷-¿ïý–-ÔN¡UNASNone?ïJ4¸ÞD?‰mÛ9?lìô†	yè?`Çæ!÷:x?"ÊS#R:?†¨YÁÄ.?ïmM{2ü,?‡!™´*X?oGûÊÑh?qæå¤úhÄ?ŒÚ¢7ØÆ?'5ÕAíã?îý/ÊË?(¨
²?€Ϩ{2?€ȑ…¢7?˜5tü¸??ˆŸ™¬Ç›K?îÛ. =¦î?t
_ª·†?ˆŽª¡U…?d
¸Ðt'?˜Ræ¥è'·?oÐéýã,Ï?íÙÒ=òKY?£ÎzÍ«¸ä?…Ôƒ7²;?}â\jÎN?¬í»`¼ùÞ?¡ÊÒÆS,?îH'2"t?¢ªJÞø¦?‡3ÿ2ü?Äƒºû+?¥¾Yٚx'?œÖZAêq?퇺¨¡¹? õJËNt7?–AZà˜¨û?¤Ä ½?¬c¨¼3j?™¼øb_˜,?í:A¸î.Ø?HCöj?™å2ëF?~öô8ڐ§?¯ia®ËÎÙ?Š9äÎrtAGN4FGL J1922.7+1428c?ãYx[O¿ÊGBIP«êÀ89Ý3L]§À9†2Áô+¶@¥¿Ü#å@U>Lò?Ê&n©«àn?ÙÂÓº&×Û@ý8bGõ?ûvýz#Ý?ëˏJ‹>¿æ2Ï˄Î0¿â•ýÍö˜x¿éjª}ík©¿ïÿRáNd?ïÆ+B£éUNASNone4? ¸‹àE?©'goE -?£æœ»ÑÂ?¸ÉìE–•·?í¶èNÞ_?»Ò°³Þáš?ºô
ÔDe`?½ˆHI¬·?Ápñƒ
®?¹{x†Ïg‡?èEB^
@I?ÀùÎ$]#ê?¼ÓäâøÌ?«3ÿž¡‡?Ĝ‡AŸ©ö?­ÿu!²ZÅ?ç>a'ʦ
?´W™ðC®Ý?xb…Ú¨4?gÙÖ¡;b?®iÚûhà?•B2Ñú¹8?íí¤VÈù?–î:´Ÿ?‹UÔµÞЄ?°
IáÉ©Å?›ÛÒ]·>'?©Ґ»b?î³ÊH‰9?µ5íu—di?Ÿ¨Ö´"VE?¦–·Ð±öÂ?Å/äZnG?Áëm¹R-?é¾mQDɼ?Â&6³Îם?²UÎòú…ƒ?¢Þ÷pà?ŴNJ/j?°úhÁƒš?èH?8`U?´-MâIÝ?SX¦"‰Öt?Hÿe¯¥?²ƒEWg?¡4%MKË ?í´CD¨?¡b¯u¡tOTHER4FGL J1924.3+1601c?éºÐÞªDã?ÉÎ81ʨÀ9uk¼ç|À:UùÖñý@ºE?Ð$›@8圧k?Ñ*YÛ=¨Ø?È.1× ì@IÄo0:?úٔ¾¾l7¿ÒñõNÌ?ï½Ë½ƒ-ǿ燊£\'¿é´ãÅ˜¿ãg†àzª¿ðUNASNone8?ÄKÚiBŽÆ?¾Äè/‡_¹?œ§ÃØü=Ð?žšºœl´?êËGUmß?Àƒ‹eNce?²Š&œz?³¹æf¹¹?³%«Ië?°Æ_+{Ý0?ëLöˆ‡ù^?¸TKD—¡¬?ÃAQa¥*?©ڳʅ:?½ø-Iu{?¥×Y,fòE?çp¥þh"?¯_|9½?´1'Á'DR?—¼¨E«?´naÔe°O?–ñ™`$2?êìÍ^~L?œ¦(Jg?·ÇË-=åd?À!à'¿t?'xÁxSû_?"UˆG¦þ?ì{@ŽÌ8?Àm"î×0?¢´F9ç£?¥[z?°Eã?»•¬`Vé?¼9xm`;æ?ëbqOV?½nmÜQz?¼ÑƒPú;?¤`edˆn?¿û~C°a?¨,æp?èfm&–d'?¯öA»úE?™µPjŒÌé?W(}r?´°ïýw';?¡†ý±Wa¢?ìœ7}3¡1?¡Ï>¾íìOTHER4FGL J1924.3+1628?àIP!f¾6?Úb<5:tÀ:k÷ÉЙ
À;'§WÈ=ò@#¾%7Çíj?ö·zU0³ý?Ñ£_ Ïmç?Æõa€ùd°?ì5J¿ì¿†?øߣ¡…KY?æt$'/¾¿ìW<'<ZÏ¿ßhŠãžJƒ¿âkÂ[YÂê¿Ù驼ÒXÓ?ȳùAI÷UNASNone?Ô)¿jþ?z?Åp¿îöuñ?a¡'Ãè(?XBKÞ1š?åÙ~·s§Ë?Å~ñþ?¹ñY_qô?ÁÂ1Žv?'›ˆ«6"^?œ/…Im–¸?ìGE^à¿?Â/©• t?àJD¡šš?´ ô¢ÙÓ(?'°D¶%[þ?‰
^,úí™?ÞOá+uñì?´®UfA†?ÒQ» æŽ?±8(kL¥?†0,€'™?xF¢ˆ?æ~a}ڇ‡?±¥½ôÁ;?ÃÎPE×ï?À]ÚYZíÀ?m5guµ?f7ãu ‹?êï6‡Y-Ì?À…Dwÿ?°p9:=¦o?¶™m*Ï?ŠëLÛk
?'~°$ć?í†K¨8݆?·"òú{4=?ÓåP|DI?³°¡¢Î?›ê½É<?Žc±o X?埮õ<q?³ß{?¡?¸ßÑw±†?¤Æó2'á?…+¯)z'?†NJÞo?짵I+Ç?¦Ö€¾wµMIXED4FGL J1924.8-1035¿Ûÿ#ârÀ(V>ò"{À9۰݂ývÀ;éü7ôc@™ÊM²o@Мe%õ?¯fõØ^Ñ?Þ{üOÇ>@>+ —ºœ@áù&Çêæ?ïé‹$£M¿ÓgÃþÇñœ¿Ý@`") ¿ß
)N­âý¿î'x_7H¿ïþ!†ù"UNASNone3FGL J1924.8-1034?§ÝœízÜ?¤Íˆ<,´?íž3öìJ?²›Ð;?§èÒ:xa?¤Lûš"?ÇÀ‹ËУ?ÁO=,'ȓ?å€'Øô?ŀ0O[»p?ÄÏ?N	?À™,ٟ;?»¤'äý"ß?¥°µ¡ÚR>?çm¤>íÜ?°ï2{'¥?Äw%•)·"?©s逾£?ÉZR9'NÐ?ŸÏ }è§ã?ÜhùÂèâ?¨lq´>f?ÖéÝ Nv}?¥B		Ê÷8?¡!ñJ
Gð?š-Ы{.Ð?í"~[
ù¿?ªñÊ#8?¥¦)²¸? ¨9΅?´½ƒ#æƒ?¶}æíÒ
?éŸ_èY+?Ę$Lö ?ÁŽÀïì.?Á)W½+D?°VÂU5ͨ?ŸÏjà?éD‡S›Þm?°=F™ðÁ?†õŸv?ªÂ̺J—'?¯J¥Üò)–?ð«ó?à·EY®ü?±7O,Ðýæ?ڑ<ºÓv?°
'$õè+PSR4FGL J1925.3+1522c?&Z¿Ô"j…¯×ÊÀ8ۚ<VÈdÀ:@æp–@òµxrW‹@´ØŸhæs?Èñ7¥³®C?Ösâû¸G°@‹7T*?ÿ'Ú7Äg?ԊÿbvAÑ¿æË ýP£¿å·cyL8¿èàyAàJ-¿ð?ðUNASNone8?ÎᕦðÅ%?Ï4|& ¯?©k¨"Q?±ÆŽŠÀåm?æ·SÛÁ©¥?ϔ'ó(Åá?ÍÜٛx}?ÄÄ¿çOô¤?·U¦öZ'?±Wâ<'$?åÓê²TÀ?ÃÍÃí«¿?˕Q@9?¶Â>y?Ã@3gÇ ¤?­ýÝb‡?äJžÕÿ·—?·þ˜Îè?®M ¤x5j?•|‹åӎE?µÞ™·x\?˜{Š§ó«\?ë_Z¾'wf?¢g6nFǟ?Ð$j ?ÑÙ¸ÏaI?³C¥Û€Ì?¶¦ÕÌÈ?å…$ùÎQv?ÑáÍxKô©?°‰J<ËH¤?´/aÅ×`?¾ÇâAÔ
Ú?»;!'öXÑ?êÚp,?¿Žhƙ`?ûúüyÒn?°]{}U¿?Åól¶Y]?±ACUwþ*?å"&Á×.?¶˜Ž­‡!?Š^¥u>P?ySžÅHæ ?¹»QæLÑ?¤Umev5î?ì_I?¥y•iÊy)OTHER4FGL J1925.4+1616?áò¶'¼)?µä³HlUiÀ8+YhQ"2À:1°Ÿoœp@ @Ÿµ½f¨@ÈÌW\h?¶DË+­?¹=§UnòQ@Ž­…èÝ?ý´ý2p?®?ÅdÞ{öÆp?ïÊSá(¤d¿äV5@Ԇ€¿çÖÔÃ;S"¿å;$,/3¿à+Žž¾Ç{UNASNone?³ìɈÈܕ?¨˜,àQÈ?{c$qâ?Ÿ˜E3í¡?ìš:óé=¾?°Ca5È?§[ÿºs?«Û›Rßl?Àp‰l.œ?¶•T±J9?êr4¯xíÁ?¹D§›W7^?­ÔØ©·ºe?›=6AZ"I?Á3åN'£ö?®o%2ܤ›?éÕ¹" l?°Ë^«Ÿ±?´s²¨ìðD?]¾ï`î?¿»hÿÑd•?špÍÃMå??éz‹Hjt?žÃ»7@a"?¯Î6{´xº?¢D'þø"?—ÖnÍmOœ?—t¶zÜ?íDi!½Ñ?©>‡Õ?ð­?˜yYômD?š^y¦í¼?Ã΄ìÓW?À|ZÓyþã?êKzùà ?ÀŒ@ Y&b?ªL§Ç†q1?•Ô´ÝÑ?Á[‹â ñè?°iPÎ}Æ?êR‹ÙS?±Ê¥›©•ð?œÝ0èÃ1õ?Öõ¿e(I?Á×ø˜
Uø?¥Ÿ<]ÕÓ?ê£R©''?¥ëš\&
pOTHER4FGL J1926.4+1602?ä;ENÏØ¿Ïþ^Õ£`À8)çZÍÀ:*{¥t@^ŽÄÔ[@úv¾£>^?Âiž1Žm?Æ¥˜*ƒ·/@
‹}ý[àÑ?üÙ,|4ÙÑ?ïhD¢qYŠ¿áhÈv%÷¿åeŸ—	œ¿æñÑiÀ¿èEþFÂ\1¿àúsÅÊzUNASNone1FGL J1926.1+1601c?°‡Ì«fa?¤¾|×/ëð?¥dÉ~õº"?¤¥n!aŠ?ì˜Ò®Qü;?°yÜðôXß?µ;÷"O?±ƒú¿oR?²"FdÁ8?§´stø¢?ës•½°¿?´õŠ˜5E¦?´ô‹–lU£?¢óQŽ—?¿ÿ'[Y¼?«`ÇÌúóe?éa‰¡˜°T?°›iZƒ>?¦b[ñúí?…>v>gó?³÷xÂ?ø­ŠÄ	?ìø¸ICQ?"ëHÖ#š?£.´'Í??˜Ý@¿6+ù?£W.Jw9Ì?¢"Æa)º?헡Øévã?©ÊrA e9? "ê¸hÌ? ° ãvC?µd×j?O?°x!$Âöî?ìJ{é¹?²;6;?°Vnj¤‹?™®هdF?¾>Î$™E?­=°-½z
?ê5»mvG|?°¿bÎN?†²'™21$?pcÆuÞ(?¸Y¸Ø?—Ò§Iˆô¬?ì"*~¦©?˜Õz˜ðOTHER4FGL J1927.4+0253¿×'¶ú†!À·tî¿eÜÀ:nš»É.À;îjCk@5w>Cˆ@GEÙþäw?Ñk€'Í?å{h÷:^¡@tu½ò>v@~?NI¿Ù|½ÀÀO¿Ö†/¤³S)¿â2•"´¿ë u¡æv¿ïÿ{Ûèt?ïú!Dô&UNASNone?ÚF…kËfW?ÂÅíÍñ?ÍZñCµÈ‹?Á^<¬ÒÃ?×òYµd?Âèá ¾o?ãá—µò?Å´lþî?¤÷…÷ÀV?£0=òâ?ÖELÙ'?Ä\~%tٜ?åSõxÆ?²±Êÿt8?Âèj0º ç?©áKÞ•?ÇÇ¿ì-?ªNÁªÀï…?èÒ>>‡­¼?¥ïèqõ/?©Œ€—Å"?Š±oµä?ÆSæá9Û?£¶î3çÉ?ËB@׶ŠÁ?»>rʀtã?Ðã+¢´å?Ã䠦ܫÆ?à½Ùø·êÆ?ÅFŠú€ `?Ów©ê…Ö?È.¶Oe?¸Àó0hòk?ºý•RÉ6Ñ?ã,!ÄÔcx?ʍxƒÊOo?Øøcêò7ý?¶€<Ë>Uœ?ÑñIQ`M{?¶Ÿy¬ ·?ÕRš™Ê?³FØÛO¦Ä?ݳLâˀ‹?³DTQêB?»#RÕåÐ)?¢0›Z7N¹?ۃÞg»j?³?1`
±ÔMIXED4FGL J1929.0+1729¿è«=Ž‰xÿ¶Ÿ_´ÆqÀ8<ó˜:õÀ::&¨á5:@Tó®N@ ,Æ1¨?ººdë<#?ÕPâC5à@ôH!ˆ@+sxó†Ë?ï'ÞŸ]'ù¿Ö«³¢"NÚ¿ä¶b'$-¿è†"Ú8+¿îDl@šúÿïÎ$ É8ÄUNASNone?¢Y^Ah{?¢©ã»?߂‰ôV"?Ì´^0šÊ?Þ2U@ÿ?Ì n4'?¦–¬Vð°?®=®n4]w?ØmpäÍ'C?Õgt$­?â_ÜÈS§ƒ?Ä`ß&IH|?¶2h¿fo¼?¥ò—ñ$¥9?àºñC,X+?¸ŸcãT?ØýƒI²6Û?¶'¼›Zò?"‹´å¶?u¹kæN€?ÐÑÓ,x^?£´ôV
.»?æúšR–?£¯¨.õÆG?Œ`ýIV&?" üU7?âd6»¨ã?ÇRC€ T?ÚTŠõ–<?Çò¾yË?Ž·'"˜žŠ?"m!˜5~?ÚõÂ1ñÈ7?ÉǐDR·ª?â
@ÜÐ6J?Éë$j‡L)?ªÿ¥+?žö.oÿí6?áÖnf'Œ?»Äyõ?Øó.Ž'[e?¹å¿cØ?nj…¿¥ýj?V̉ïw-ž?Ôëðñf¬?®b;Òq¯ù?åk®?®\§p¨ÑÉMIXED4FGL J1931.0+1754c¿ïàõèò>ĿӆoE],VÀ92ð¤BjÀ:‡4éد@ê''¸@_Ëâ˜@(öÎþÖ4?ÒÎBXõ»@
…凮¶@öˆþð?ïë@öjU?âA¦=—¿çuݜþ¨è¿çdœ,ý¿êϯj¼6}¿ïý "DsUNASNone8?֙JÂy•K?Ék#U€Ì)?ÓEñm"Ø?Ð:Î'jÓ?Ö! LåÞ?ÊÒzoÃî?¼1BÜã41?Â:©ûwÁ>?²à->áï?·æ
OCÁ?ê7»ž"Ã|?Ä…2¯TÂ?Ò¡JE&-?±ë°‰®?ÇJÍæt¶?¯"¾Æϲ°?àÜÊa@?i?³¤ÝP,Ý?ÉäáJ:ê?»RÐ\yR§?š2nC'è"?¨0ýYú ¯?èµdՆs'?¼´¤_£Ý?ÏoìŽå?ÂîW…'¾ž?×¥ºÙI Ê?ÐGå(ۍÒ?Øэ0ª—Ä?̃Յ`°?µXmý7?½×¿d?º$«ÆláU?ÂRU¯¬Lò?ê\Ç´½•?Ŗx"ˆ°
?ÅÞ=M'd?¨y¥RGf?Í%ô:ó?³aHÿ<$?ãH'0=
?´»xˆ‡5"?Ã=Po¦xr?Ä΍µ=l¦? –G1®Z?º"™vrÿ?ê'Gt*@¾?NJh+ëô¹MIXED4FGL J1931.1+1656¿ã1 °}ûr¿éew•ÜvÀ8k§AøÈÔÀ:£ùnì@é'"§ŸÂ@蓂(cÌ?¸3žèãÙ¯?Øf¨@%‰ý@7Ý÷vÅ?ùõzÞm‰?ïÕM9Æö¿ÝËØü0Á¿ã£˜ ö/G¿é ÝDU¿ío³íöz¿ïàåõ"UNASNone3FGL J1931.1+1659?Š©}[X<î?‰§H°?ép/¨U?Äm$†9G?Éó§n»ÁÚ?ÍaÁªÉ‡?–Ð=¹½ñ?œ½èyÊå?âx©cÞn,?Â%ÛWEï?Ù¡©\t	?Â#эÀ?¥ð´Á«@?™ž}ÓGR?çOedÆ?³·ÇÃÀ¸?ÍFb˜?²d¡ÑÓ©?'7³'ôE?cA¬£Ü›{?Û,§ÜþH?¦–üõHÇ?â!^í•?¦ºõ^çA?Ž¾®e©^%?¨ÜOòg®=?齁›©œÐ?ÃB(][¼?Ç«5ðŸ?ÁÏç^s}Ñ?["0^ì?ˆ­BŸ¶þ?ãÌ[§Šb?Èü%f½'?Ùc‹'x<?ÈÑO"€?•2R"U?Œ6Ÿ¢'Ô"?é—ŸþŸ?³)Ý/VÀè?Æý~:Ãu`?²9Ÿ9E?^Q&ËïI?Etd'5H?ޞ¾±?°÷×|(E?ࡈ–<?°û
ï˜-þMIXED4FGL J1933.4-2711?ì€å¿Ñ«sÀ4§ã\[J©À:]«p_À<€»|Bq@k"§ïó˜@)ô?Ø]$?ÈÍfOÀ1´?ͪxúgº¤@à±5—''?øÓÁñQ'm?ïøU¦P¿äó~¢r[<¿ê_ý@²ø¿á'–
qH¿ïûÚ×Q‹
¿ï`낚y"UNASNone?ïkÒOÝR?•x§Â¸]?~PõŒÆ¹Ä?{\²úZþ?–~HJëb?'šnó×o?í"RéÃ
í?¬ÚY?Ž?¢è^™Þü?¦LjêÞÜ?£â¹5B.?›g{Ebä?í|A1×8?žÊ¡ºªS?›‡C—Ak?'õàcÏՍ?ªx]Ä2GÇ?–B܉ÞY ?êê=ÿrš?˜"´«­h:?µâ¥6#á-?'ƾùG?ºÜâ2~?@;uí…?íS'7¨ìP?«¨s¹ ¢¬?"÷‡jÕÒS?'Ïwèh
‹?°%"iMe?§ƒL¼v\`?é•"£
?Áž±¾Jö@?¼ÿðX˦»?»!Ó¾Mó?º»cÏ@ß?³f´¼ä(?ë3X¾Ìȵ?¨b]@˜Ž'?«×åÜG§?ž :=U°h?¸ÖN‡}…?¡'PÎ8W–?â¡~"r?©RlÇDä?ÈèÜU‰|ô?¨-+ùVo?̑+:Z2À?¤]¨ÑŸAGN4FGL J1934.2-1446?ä(_»ã«À0!BoçÀ:ײãâ"À<]՞,¦@KßS75@ôK+w}?ա‰?ïúºEዡ@©¿f²¼€?òJ̌¶b?ïûÂ^ôÆ¿âI†[Ï¿âp&¾°ªW¿ïþª_ºz»?ïÁ5Ø)!¿ÛèFۆ£ôUNASNone?ìÎâW3Ôª?ÅÑð‰P²[?«R°/•ìQ?ħy8ži?§¿*_À~?²¼¤F×ç?îõ%["5?µrië0Y?›Ü'~sÄ?ªê³w6ô?¡òeˆ'Ë?ªê¥×"ÅÝ?èñY†Pˆü?®‡X"å¬?³ˆ(ncSð?¡…"€Ã?Âv…¯ú%˜?©]µyàEï?ì)<¢Êç?­W‰«oAó?¢ì hïò[?£OÕ}»æ¢?µ@
»}–š?£}ã¯?ì¤éÓd?¿BŸ]O?¦m¾iD­¨?¶çAÁÏf?´ù-3Œ?´ƒ‹wÆIÌ?çç›ìÉÜ?Ï­¸=&Z?Ș,(ŸS?Ê=ø‰¥A?¹±ðA_à?¼ûË
Á÷?ækñ'ä¡U?±ÏJ¥Þ"?»ÿ`w'îu?¦ªBµçjù?ÈP‰¸Ùƒr?¬éù™¹˜ö?áD&>>eR?ÆôRÖDM?Å^í(ëd?ÄúHí"?Òõî¿«?Á‡Î§)AGN4FGL J1934.2+1036¿ïŸÔì½Àdf±æÀ9ê¡/"À;q¨žð@u+'SO@êÓ²š?Î8×!qÍ?̪'».å?ûìÓi©@Ú!« §¿ç¼uÁù	A¿âŠI{õ¿ç«Úy]¹ï¿ç!¯}0­G¿ï÷ä]b0Í?ï(ڟsMUUNASNone?æ"Њz ?ÁCmÌûàz?ƒØ"v…™?yt9¶K«K?Ó0»kü?Á#Ntq?樊et#?Ãh̐DŽÙ?†+èó[×?Š"d'Rـ?Ñý‹íš³Ü?¹AVÙÍß?çΧž°Q?¬Ì2¼ùl©?¡áâ*?ãV«?|?ÌMˆ.À»?«ª#êëƸ?êš4)Ñ?¤íÆý¶ì¿?†oT!‰?kvdgˆýL?Ä0:¡LÒ}?¤N,¨v?ØóU€B¹?¤¹¤7=•?'ÐJ÷Q?…'ÇÅüÎó?â÷ÒèxWˆ?¾y@nì?Ù÷ë)ëG?ÉÕØlÆ°\?'&w·<YÝ?œ¤¯<è†?âzÖ­B»3?ɒ7߄#U?Ýuÿ¬Ú$_?³Ð1ú™¦¿?±|';ìÛ¯?™.?uº+?Þ*ßÅ·v?³î¹5ñ?â‰VÓ¡RK?¶ó=iùá?˜¾ÑÀE?…;à°ù?Ùae<½?¶¢ÉZÉǁMIXED4FGL J1935.0-0553?ØOn&oÀ(¾Ÿà·öÀ:(òvªHÀ;­Ëwb7-@^R 3Q;@Ç>
&Ê?ÌVïûÐñJ?ÉÀœþ('?û)¢á@ø@ÊQŠŒ5ƒ¿åu¿äF¼¿á"՝U漿êú©]\¿âSÓ¡Ó#ÿ¿ïÿÿ" 5•?ïâÞA>c¾UNASNone?ïQ~î{%ï?a•ú±?0?qÜ*ÛoUº?kƒaOwuÑ?'Y{û+¸?Ž/Å•ø;?ïN?"¿?™ìÂÞÿƒ?rΙBÁ!œ?}ñ5í?'ŠñÀ_½?– hý°Ê'?ì; ®î?¢Œø°Ý+_?"çvñî?‹	_Û?´'•7`ôŸ? Ct•pm?î54?LÇ?GŽæ¶x?wssќ2?_MU»Î÷?©¾Mø''?‹Gî?Þô4?î–ä÷¢µ? Pq¾{?‡á·‡Ä™?ƒÀ×Mꦠ? ™B¦€£M?›¹ˆ¥Àb?îM%2ü?³šÒ`?‹"*³¡œa?œD H(p‰?¨É°›1?° š+‡9½?éݚzj)?°c£,Ú·?§ËrC,?™Kƒö1z?Åù­!zN?¬Œ¾ºœeÕ?ê<¦ÞjrÔ?©‹Ÿá?''Lž>D?€^F̀?Ĺ²=ÕM¥?¨5…ÚU¼AGN4FGL J1936.6+1921?ÎôÔÞi,i¿è°IáÀ9"+zMÞÀ:µ®Ò­@Ù£‰²pÖ@€"Þ?ÉSàQäÏ"?Ì%=§*{Õ@àÌ¡-â'@Òÿ–ÎŽ?ٜ߯}‡?ïùRژg¿çÝgNòr¿æj}2…
¿ïþ;·f3?ï±<î×íUNASNone?Òú̈́z?Áx/~?B'?²¸ h6g?¬©•`?äBߕ?F?Ã|Ø\'À ?ÑÒ9HԎ?ÃÏF0Š?µ(|7«_a?ªÏ±'±ž?äqï\ªáý?Ã;ç'
ã?ύø¯1d?°ãJ'¼$·? á+Ôo.?¬Ý¾ð<ÔÍ?ã"I‰Çû"?³›e£R<ÿ?ѨHÓ`ù?ª"<×Y•3?Á^cò‡‹>?Ÿ£.vhš§?âÔBšY]?­!4«¿r?Êé÷wg¸?»hu_S?·LU¾Ú?²þ{ô}?æaØÀ©†?Â5ààjc?¸ë½«?µŠø'á9?»‰
øxïw?¸uœ&ä0Ç?éŒ!@8÷?À®rx\U?ÁäæFùí?¦7*çÚ@?Áy5=t?­2Û'6-l?ç("àò@?²âÆ?\:?¸$où®Ù?ž¸gŒ—ƒ?Æ螫b€?¬ÝrÙ÷|?çAJUÂ1ò?°_‡YÑ»OTHER4FGL J1937.1-0444¿é5K±Ÿ†À(¥îÇÉXÀ:§
ûÅ<À;בÕùµ@ŽÊɽMÔ@Ñò¦{)l?ʞ#×u;?x	‰k¤ï?´!ˆ¬6@5™ ûb·?ïO5'‰ ¿ì¿ôÕ÷¿âѱkë¿âLERðgÝ¿ß=W´¿ï÷ˆ—é–1UNASNone?îN¾
¹ži?§"¥§®€?^±Ïޙ»?Yªµ¡9s?ª–xdÜ?§O
^?íýхª_¡?±8¬P_ѽ?qÑvŒµ²?{VÔØðT?­è¸Ñ_B?°¡ðت,?ìօlTÖ¶?¢oÀLÖN?‡9»»ìû?"w·*ÓÛ
?¶YÍfOÀ2?¡¸af'?ì\Ÿ¹Kï?'¢ªÜg?nWî"O«õ?R$/%"¹V?¼(BÍ͢?'Wð!¨«·?ìÑ«ÄА?³e´'aU?q½ÍV8´?hÓÇBjLì?¸[}Ë7w?³&îŸÑM?ëh–¬KÅH?Ä{4ÐRy†?{©QO)f?‰ÛÄG©H?Á€]ã|Ö?Ä(´›
ô?éÐvÏâxR?­ÔáÀÍ?"YÏhÙ>g?Š¸ò"½\Q?Æ2êÒ¶	¬?¬|Q`úÿ?æ0V‰új??¨œý®q?'"Íæ²?pB€â¢NÚ?Ó<}M¢d?¨>®›Ç6ÚAGN4FGL J1939.7-1242¿³ä77ÿ¿¡À0`À½ÊÑJÀ:OL{ٕ2À;äñ"«=@ã7sá%@÷>^‡?Ï"/)ä*?ԏ=?{•ø@VÿëJ?òoðJÖ=?ïá·uL³7¿ã¬u:'Ä¿éb†ÝÕ2Í¿åãÈý4s¥¿ïÿÕ} i¿ïä×»=XPUNASNone?ìyöÕÏ?Âüp½‹?­V¦
-dï?ÁR!Þª£`?±L',†?«–*ÄΎ?ëáôM‰¡?¼Ëç8w¯~?±å²Ôï+?³Ïaˆl?®U~kþœ?¯ôA–.r]?èùçá??¬f
 Þy¡?©Š sÌ?—v'G«UÓ?Åڃ¼?©´­*Ìۆ?âXxÿ'"9?¤Sàû?Å%ëÌí.?Ayòà2?ÐÂ{	á€8?¡ë}F?ê±`äW""?½©,oÛÁ?°ëe''vM?·A¸îœËë?¹‰"ZBõ&?±3Iy2ÖH?åS>'¦¥
?ËA™:ןí?ɱý­Y-Ý?Æì~
LÝ?Á=ü?½Z¯A)H¬?åúù€Lþ?²¤À"Ò'?´fôé'ù?¡pü¯¡H?Î
èWS	N?°è…èß=m?Ó:C§cuŠ?¦,'³–?йà7¶?¬,xÙÛ~?Ü+xdüÀ?¯Y¿œµUMIXED4FGL J1940.2-2511¿à¸û-՝£À5[«!ZÀ:61•¤A"À</Æ|P³w@Œ8ê8C@ZمAóÀ?¿ŒãÓ¤'V?ЀhûÂÄ@·»Ã
@%£fÌè¦?ïщàiÝ¿»Ž>Wå«¿ãi–!!Ë¿æö.Åæ(¾¿æåP¡F6¿ïÿÿ" 5•UNASNone?îºpwÈtµ?"ÞÇLåsÓ?Œ"´Èº'?ƒÈèGlÈ ?š –¤Kî#?œ¶Wð?îZYàœ'?¢›"dž?•Õ™Ž¬·¡?•¯õ6ßvY?žß*aARJ?—-†N'?íbõ‹»h)? "bÑ<X?ŸhÎÍIÉ?"æŠW5'?ª@<+
?–|Íyæ?ì<[®…?Œ-æ	1&?¦uŽ€":?3^¦zdâ?´ÃUá¦&/?†¸,›ƒB"?êß Ô~û?´XsMn"?²Y[Œ©Ø<?¨Žà^ù*f?¶­ÿjŒnk?¨[P‹BDÇ?ëÞ­'?»-s'ÙB?²¯æöLU¢?´.K³UÚ?´Ñ# MzÎ?­—Õã戤?éf:y¡?¯´˜×'¾?¶™j-ï?¤²ÂˆÆЙ?¾4Âu ‹?¥O#1YL?å;Ÿ­?¢Zé«`ޖ?¾(~›³Ç?'o¿'3%?ÊïcÁ¦D?ŽÞêãbAGN4FGL J1943.9+2841?͛B­	õ@!‹zՉÀ:—{!ŽÀ;ú¨(÷@UÕ¢ß="?ÿ'þtå…*?ÒM£!Ø?á÷Ix@æþ*¼l?û?P"]?è¤zÏ)¿éS-Ú-Þ`¿Âë·sŸ4
¿å0>·ç¿ïûêAQÙç¿Þ»k›¯svUNASNone	?å)'ð,DÏ?Á`ç‰Å×?¨.÷y? Inöè0?Òª"Oûs?ÀLýNIº?àÅì£?̈{Cît?´
Ñ»m*°?°~'X}?Úý;}_/?Èô^®ƒ'ù?æ8ì=³ó@?±/±mºó?¸_À#köæ?£xôFYÙ?Êìnø$Í?«'Œ>z*?áse'w?¥Â€ QÙ6?¸Ç®pdn?'œµûŒ?×Õ'J'ì??¦âíEtE¦?Ö§]ãÏ·?Àݑاmå?¶OAWâ_É?­³?áâ‹&Š›?ÂÊgæ?ÍH}Buñ?ÉÑ)Ú*>©?ºöè9?º+©ÀÇõ'?åO!ŸH@r?Ê;ìͽŸ?àÓOrÙç?´e*}âA?Áݼ
çÛ?¬mz ½ÌÀ?Öó{_XD?±õum­g?Ò!H#+ÿ?©ÀE~Ì?¼«)l""µ?¢?ʸxìv?ãYöÀÞyj?°'´t:åMIXED4FGL J1944.8+4301?Ã
Á†êâ¯@"ˆ^	}À:ߝcRµ¯À<®nƒkYë@š7›Í¦?ûewS´?вï«ôæ?ÝßÉÿ'ò¶@
°Ð?Hl?ð\^š/A¿î'@"ªt?ïý%Ÿ÷¬Ÿ¿Ð×L¶8Œ¿·ByLG+c¿ë4rÞn೿ïÿþ½à ¿UNASNone3FGL J1944.8+4300?åa¥~vŸç?Ã#*Ø×Ù,?ÁØO|~?¹tÇT_J5?È¡•æ?¾‰ôÇ"úè?Õ+?ʛƪK?Ö©JØ*à?ÇíÚV«»ä?ÔNŠê ½?ÆLäùÙ?çþ6BB€ê?¯¹±ÿüUû?½µ%wo?¦¯L€®ˆ‹?Á{ß=#?¦¨†¨muc?ãàYþ½Ïs?§Pƙ'gð?ÏugáÐ?§áA~ô~w?Ái"'²e?˜«…þ|à5?á\‰¼VÞ?Ãt÷R M?Ë#¿W™D	?ÀÉ4š$?Ïlu`?ÀHÌ·ÿ
b?ÅÞêú'áL?đÃÆW¬~?ÞäõÀ†d?Î̙Ũ/"?Ö+"´õ?Ë*o1Òz?ä»$¯?³ë+éó@?ÅfD5A³Ý?°mûy•?ÊEœàSšå?®4šI>y?Ûê^È:?²JQrÑhD?Õs§v?ç?¸¬ñh-?ÍD|Wz¡m?¬Æ¿'ÙÉòMIXED4FGL J1946.5-1527?îÕ}J1IÀ3ªCåÀ:­;qÆÀ<2©ˆúåå@+QœU@MdQ¹08?ÌZÂl½?ÖÂ{»[@û͆00I@$_6œIL?å*zAå}ž¿ØôKâ»'¿ÒЖ‰B¿ä¶ÌR֒¿íÈi[
lпïÚ/÷>_UNASNone?êºÒ{"Ó?±Y¿)ƒÙ?®¹j¦YI?¡°N¤Ä?ºÌ¶Òd'O?¨»±ü?în/žK?¦ôñ_WÑ?œœ†é%¹q?Ï̪"Èâ?¡ªÚøs>?œ³ªe9'½?鎼¢Ìâá?­2F!˜J?µû¯"Ù¹?¡©çõ£?½ŽkÊö«:?£Æ·5Áù?é;òVk"ï?—gB"r`?°îé?‡ºúQH:?Ã¿¥‹¯?"bÏFébI?çio	D™¯?¹pAɈ?¸Î5¨dà?¬Ñš»Ÿz?Åó)MeÓ?²N4­_3?êȬùë
?¿eaXµxÈ?·û;Â
(?¹Øh"òt?·nš…?±3§>#Ð?åu[ÝT$?´x;2"t?Ã"Q¸ÁÊ?«±Ä'#€#?Ç>ù÷
¤?­BëÉ""v?á¹ÙÚɲ?§Ì"†ðœ ?½˜%³XÛ?žÉG4±ˆZ?Õ&BÞ»¦y?¦"%ˆ¼AGN4FGL J1947.0+0031¿á@–wj¡À(2¦Òg@À;KÍ]ìÀ<±
À¾¢@Ͷ˃¡‹?þˆKBôqW?ѧ+='¨?ãŽYM= @º2nU"@ìé‰ò?ïõ-¿‰?ïý¤ Y?Ùς‰²›É¿Û®âÛ¬ä¿ê¬í3t¡"¿ïý4©Tø€UNASNone?縨DšÓ?̌ª¬Ö&,?£fìô
?Âm{¹3è»?¼ô²¼LÄK?Ä@DÅ)‰?è΀ÇnF¸?Ƽß=""?º0w4Gç?¹¸U[ýò?¿['F<X?Àš'
ÅKµ?çç7»á¡?±€oûžC
?Å)žvšˆy?­$'	?¶tÁT}î‰? àIã@//?è·cK \8?§ÖGßbˆ?À•v­†á?£ðÑöY?¹ù}|Ný?™Û£¡§§q?çCm<\?Ææs‡6?­?Êk¦Ûæ4?×<tFñ#?±
Hgи?¬ã\Ð`Ï?ä"úû"9€?Í|°GäxÄ?È¿4܉5ý?Ç(Fñ2Ö?Äðß6íä?ÃQ<¨Òǎ?ã<•Æa‰ï?¸jô"?Ðágç£pf?¶Àu&?ÁJÙX¸ö?§2•›¶"ö?â0¸ºF7r?·MQÝçS?̄Tá·H4?· (QjÉ?ʸÈ3
ˆ?°SÀ·äµAGN4FGL J1947.1+1729¿Ã˜•£íxÀËEˆ MÀ:~]yWÚ²À;ïpx8 @YYJt@ˆÞ{Jùù?Ò¢É4<?à®
>¬ãù@&Á» ÒÞ@ªåq^?ëgÇÅ&^?ïÍýº¿Üê¥OÛ5¿ßŽØ'?Ù¿íÃÌ"'áÇ¿ïéý"ë´ïUNASNone?åG‹"ôk?¼§ê®ùÁç?¢ë¼º—?–ƪEy·?ÓqRcá7?»g»æu•X?Û!÷Ȁ|?Âå;:‹
²?¥9ËE?¡Äü‹¡?ág˧o?Ž"²r?èb•ãpl?®Mérú«?´1iv¿Žœ? ®ö°Èuª?Ä\ó¶p"é?§7€0þ)Û?垥€éŸ?£n	t¨0|?¼‰ûR,ƒÓ?™ú1¶³2?Ë@lXæ™? "mQâØ?Ý9V‡dýt?À•Æ`zÐ?µ8šs+?¦«AY3?Ýx'ô¢ºç?Àvn©Æb?Êe$"V[?½¼F#È(›?«ì'¶yæ?®¯i7»°?ç¼Þ‹Í9j?Àäÿ3UB?â†|9–º?³X8ס?À=ӄ:Ñ|?§z'Içm?ÒÔɔ‰?°T§rÜQ¶?ۙkáÐj?®«ýê½?Æ°A*0™ë?­$/)ü7O?Ùsˆh<?°
à‰MIXED4FGL J1947.6-1121¿é­PÚ|Ò}À1'à°«À:&whiÏÀ;ñ"ï¾i]@LAô—2@÷T°[|þ?Àò1uÃÑ|?ËÚ\S=@áÝBeÖ@îa§ºÅ?îúA¯Í¸…¿äÅïbùÊ¿ä˜zJHùn¿ä¶"¡¸!¿í6A
çI¿ïÿï0l¯UNASNone3FGL J1947.4-1121?èMi ½š?¿¿æŠc?º$,<|`?±˜ÇtŽÁP?Á¸CaîKf?µ"D˜áN?펪˜£,?­HWL?¢rDMh½?¢8ؤ|"?¤£74òƒ?¢@Ókã®?ê'U¹'?©ÃUý#?³9"éc? ŒXõVÝ?¼ªu/¾è?¢ŠTrÂ?æ¡êµò?š#""±Ö?µß€kÇ?‹®U…›õ?ʌaödÔ?–Öf2­²?áüèm‰'³?"ȳá?Í9~bÜ¢?½œÊâ£	?ÊÒßçÂؓ?¸Ã«6k?èÞ`qþ?Áꖲð"ã?¾Ö"!¤Y?¼»È²O¸?º6ï€Uûµ?³[5/â›Á?å†lí$lW?²NyØۏ8?Á¼?Ù½T?ªÔ¸!Æ®Ž?È)Í"'P?ª\tǓ'?Ùò¹[×?£àœxÌ8‹?Ç-×çæŒD?¢öýØyL?ÚvZ±¹?¤°šgó
MIXED4FGL J1948.0-2845?ä¤Ñ{ª"À87÷ß (À:Âôí}F}À<'øxLAø@õÉ¬²@ÝӅM²:?Ҋä?Z2ü?ÆÍyÛc='?öéjâÌéR@vMP¦?ïó÷H¡Y¿èM!@—tÑ¿Þwgà¹é›¿åá*È*§¿ð¿ïýl§ÉEUNASNone?ï%ñ0¯J[?í}ëW?rŽ䖎?n.mXúiQ?–ÁiMhÁõ?4Ý dËó?ï}ÊAñ?†^í'3–H?jV1±D-q?qW­x@?‰÷ðŒÑ|b?šžrn?îdÈý?–1F½1?"gÃÁ\íq?œ´õù="? 
L@<´{?‡%?îW@/èGt?cÒýaÄ?|]	óUA
?\ÑÎ1Xj?§[¿uI¤?€!z6?î"w—ÍLá?¦
l[:;Ð?ˆ=|'k¶?…WÛ¢íD?§Öw –û?¤•p;?î˜N•[¾º?¡G¥÷«·?~·Õö›þ?‰ä€¼‹³"?¢¤%@à?›px_£ƒÇ?í³Ÿ²Àæ?¡¬¥7BÉ?Ó°¢¼ÜS?"j9ÄAÄä?¯í°á΀?™±-	""~?ì
"²­o?›!yy
B?ˆç	‰Íð?u£8ÆôZU?¼'J/yi?™»‡ÐÐYÎAGN4FGL J1948.1+2511?ÕT÷Ëu.¿ÆÆ»üXÀ: !}(IËÀ;ÎôX,@ŸR–$ð@L¦¼—Ëc?Õ¶?!}ÿ	?ïý½À•[ò@Ö|^p@'ܾ²X¿îêÎà£Cg?ïƒP˜È¹¿ÂTR½'M¿îAŸÀäa¿åË@¥â}8¿ïþ½_ÇeÛUNASNone?ãu»¼ë>Ž?É!/|¼¶w?À÷ ¸N´?¾ë°Ó@?И¸*ۊ?Äÿ°ÞÉhX?ÇÃ\Ÿ?ĵ	)ÒêÒ?Ãd")öt?¾S¸¹Å^?å6!oïÚ¡?Ŕà.Jãu?áâÇ*Kƒ?³/ÓWí?•6!hõ&?ªÙyü—Öü?Òï֚´W?±D¨àx??ßø+^J?°p¯¾¿±?Ñ»âC×p??­üÈ>Òá?̘!"‹y?§öC°îp?ÙÓ/}•q?Ê_Kr¢½?ϲ¶q?ǧAbuëê?Ö¦÷§'2?ȦYŠN¼À?¶‹îÏð²t?»«QR+S?ÌK̍ô?È¢lb:?揚l±?Êße‰OR+?Ü\Æ~mÝî?¶Gæ$ûõ?Æ4óo×[û?¯­mÖ°?؈¿É¦t?¶Êª†òe?ÌàöxJr?°æ?HA´?ÛÞQH`Ü?º"ÌiêCD?Ör¦r'f?¶öxëï¿ÐMIXED4FGL J1948.9+3414?í‡óç˜Õú@ùÉÕ¡‡¥À:Œ%ÿnÀ<d._ŽÛÐ@€Pþ .‰@'ƒ$ã?Ì)FNm÷?ã$"¯&ɘ@4·|Ùor@*¥"8äù¿ïþ1ɦ§Ÿ?ïÚÚ¬‰`f¿Ï®öxçù¿á©=¦~¯¿ïÿ›‹â ò?×Fë¡Ï4UNASNone?֛Úa4ù1?Âsn‰t?àBg¶?Ãýbì´HÇ?Á¾¬eE¡l?²Ï©ôŸH?ØéëØ	Ï?Ít!ý3?ÏíT›|Œ‡?Ʋ.Ä˜î?×iÚ0¯î?ƖÌ⾞?ÜÄ·–ï?µ4"'"è¬?ÙÕ¬'na?µÆAÌHÛv?ÂË8"ù?¦ë(Êâ.?éžWS£ì? XN|¿ã?¿këq¹¼á?š4ˆ\€?ž?³¡YóL¤…?‡y›\Ÿ?Éï—èi‹_?¹MZå6£?á¬x'Xño?ÄÊ·Qn?Ï^†2®å?¾¸ìYB"?ÊyyRtu?Ç#ãH ?×ÈïSp¦—?Ì sÄY?ÚúTæ.?ËH3_þÃ??Ì󉭛â¨?²zëê<ò?㏉
7ÿ~?¸í9"Ý]?ÄÎR"_?­Ú]¬t
ë?â=Aô«Ó?®lšáVíY?ÐB«Ðl®C?­IY¦#;?ƅ£ßSô/?¤,wÁý~MIXED4FGL J1949.2-1453?ë
Ôæ±À3c 1ί%À:9ìTRÀ< 5)­x@584¤ÍT@º®ƒ?Â-æ˜$ú`?Ïç™Â3k½@
®Æ±@£'ôf™½¿çXJCðñ¿Ö·_þs¿ã
çŸïõ¿ã9>Js¿ï¾'€p}Á¿ïûúëÄ	UNASNone3FGL J1949.5-1454?ìÀ‰â0P?®o.ø@7
?®ôoq/ µ?¢&×Úi?°'ÃøV­%?¢¤´Úܒº?ìFoÚÃh?¶ø?ÔA»U?±7ªƒa¼?².oŽŠ?©)®>á?£¤ O8Ÿ?é0¶øéÐ?¬†#)3?·::ç…?¡Ò>&±cž?¿]§Mj?¤¹§$Hi
?èJyÒà˜?œ³¥`+¡µ?¶oè×U£?'ÑŠ3»'j?Þ$IF¬?—¥-%Æñ¾?æˆÕ¬o_3?½¤Çù?ȇIÜön?¸ŸeÎuu?º«0ˈ?«')½þ"¼?æ{Ϙßé?Ç"塸'?Çá§å·ªQ?Å8'яµ?¼^3kV)?³ü70÷L[?äjØë,øö?³lÔÅÌ}?Ä>\B\W*?«
£??Ê@ïÄý?­Êw78?ß>œJwÈ?«"
Hñi?Èÿ׷Ȕë?ªiVVŠ˜?ÔAwÚ=Ã?©Ñó¸€ðAGN4FGL J1951.0+2523?è:ÜÀ"a$¿ä¿Ž‹HÿÀ9á8ˆÝ‰³À;‰á<ÆYì@\fHß@´±'Äjþ?ЅÁ?ÐÐh?èlŠlÕì@ûà\÷R@½çMVŸõ?ïðäÚ	Ì2¿ßöP<Xv¿Ó&íàBËW¿ê»Á¬Þü¿î*GÒ&©¿ïü UŠ÷UNASNone	?²÷ãWcû8?ªH"NZ?Õ=óIÒö¡?ÄÅjHÚJ ?ã	ïåM?ÅUñp'†¢?¿bdèÑ©ð?¼"¿­TŒt?ÇJ¯j€S?¹)"øðÎ&?æAˆEÅm?À/Τ¾:ä?Íüw6«|?­©²"V(?ϵX"<&2?±b ?à"Œ)C›5?³½4ßrÑ5?Ç-Ϥ¡?œJ»ë%ø?Û¡e £?ªìçö#&Y?ØÜ
œÔ?ª˜;ðkï?¡S^K	Ê¡?•}"h™—L?Õcà	jŒç?ĺ
BâM?ä8ÚŒ^s?Äÿ=.Öúp?¢Òj`P`?¤\MBYêù?Çw^¾ÔÊ?¿ñ§•¹Bà?èôþyî§?¿%Æãÿ™S?¼žûÝuU[?¡œø#á³C?ÐÍnT¾À'?¶<,?[Ý?äiYñõ?·Ù\ð·[Î?¨<»…ó6¨?Š®þ(™_?à"šö½i?³¯ô›e$1?ÛÑ2¡´9?³Q7v¬DMIXED4FGL J1951.3-8015c?í2ˆZÀ=;0aǛ5À:P,á	š³À;þí¢/jQ@p*^£N@(ô€oüè?Îå?	U>?ÉsN@Õ³%?ùи´çÓ¹@Ù1΄1þ¿è"Xº¬8Ù¿ÞNvZ¥=¿äÂAƒ-¿çÜzŸƒh€¿ïü»ýǖ'¿îì:ñm–UNASNone ?îÚÊ9Z{?š.?ªü»?x'g	õ-[?'PQÅN7?ž'$½6D?–øÑ(Z™?ïbˆ§?/Ò?Œ>ÁƒXêœ?mï>õÕÙ?qVÏ™?âll?†œ÷æ䢘?î4ôm>Œ?˜qƒÒ'F…?‹àÁˆh?ƒ£ë3œ¨?§"Æ6Z°?"¥œžì?î/ðéÀ+1?'·Z¬Qð?ƒ?Uã5?cögæÇ1q?¨1ÿ*'%?€í¦–ƒ˜?ìaU¥xŸ?±EËï'?'6ÌÄ	í?ˆ®ëzã;?¸§Ÿ¤r&?°ê4txc?îŠz( l?¨ÜíQ2¿É?ƒá¾œîmÈ?Œ'—•àø?ªÎèµ$~S?¥@ôÁ!a¾?ë*—.k‰w?¨LSX¬9e?¢¶bÐuG?"æ¾éÉ؈?½P'j¹C?£ƒÒù{p?ë±´K`ž?œœ—íöQÑ?"SÙf¦6½?q'V™?½iƒyâ?š'X¾Åé}AGN4FGL J1951.6+2621?ï{Ã*?L¿ÑTËß<'À9=kŠ'•™À:ÉV¸syt@‹ž[JS‹@ÓQùÇכ?ÅÔ\c-L?ÑÀª?.>,@U-úNw@#^邏?ê_åBåWÞ?ï–Ï)ž_¿âcž\vù¿ëN
>¬ãù¿çüÎR
¿ç`oâ*ðUNASNone?ÐÕò™û?ÂhÁõÙ5'?¨ö¥}p?¡ònvDÍ?ægŠl™Ë?ÃáëY¢*.?ÈJãˆÐôz?Á§Œó35?º¹¼®$?°¬í{K®?æ¬/û4-?ÁmyWQB	?ÌàÖ,zò?®qçÈØtÁ?ºvՒvÃ3?¢æ|º$yh?åxï'ƒ?±A€€ëc@?ÇÈb¯Í'? %U±Ú¥u?Ê6®:ÃþÑ?¥ž½•®DÐ?ã€;Å[œç?¨¡ Sf?Ç+ÀÅyé?¸|y˜rR-?®n¹êæ?§d5yRŠ
?èN.3šú?½±Ú°:E?­–׍(´?ª·¶'at?À,
5Xã'?¹³Eìb-6?ê9æ£?¼!ª—H?ÀÏYú?–?£ÀŽW2?·¡`em'?¡óX×Ñpr?è×ýtÔx?ª—²{Í1Ë?°gcËpE&?'ÀoªŠ~?Ð_üe§àÀ?²Q§Fé9
?åÃSyNË?²n0ªLcOTHER4FGL J1953.5+3841?ƒ룝˜ž@¾Ès«ÉÀ9"w3"«À;Á15,2@¾á˜5ìK@žŠdrp`?¿ÈYök®?ĽßwŸI?þEÀi;'@;1KýYˆ¿íª¬çT7?ïô"&"À¿æ¬Žhãï(¿ã¢»a—è¿ëVœ_˜¿Ö1q<-WÒUNASNone3FGL J1953.3+3847?çütÑtb?¼Éí§ìKK?Ÿ‰Ó[ÑL?–E|ù3_?ÌòOÏ\Z?»¢AÖ0› ?ëV'B1u:?º'Ò+?ŽDøœMAì?"jVe0i&?ÀÁ§lbv9?¸)},;%?êÙpÖú®?§eßç]|?¢
U菬ù?"¨a$áuv?Àç*ϕ?£¤…¼7#?í\ßâ?‰B³%7-? aäæ7ñ£?yåÇte.
?­¨YøZIl?'½Èç©·?ÞúPR¼õ?ÁÀ Ç`?¹ C¾7?°È!ÂG³?ڝž¾hþ>?ÂÛNxf¢?åBÙ³²kð?Éh%Ê%8Û?¤™;.b«?° ¡qe"$?Òç%2êc?Èä.Nƒ,?ä…u+,?³lÁó§?µ*x'%g?¢±å²û)&?ѱ‹Tÿ®?°ˆñ,õÎÆ?銬t,f?¡‡Eü[?³"•³ú?"š|‡Sà—?ÀD	3€é?˜¿0Š"÷AGN4FGL J1954.4-3729¿îQœÞP6À;û¨`ܹªÀ:Æ(¯K²†À<=b†ž@åXvc´…@áhšô­?ÒùYÞÍÒ?Ð
Èâ¬?õð ŽëÁ@±:ªËÆ¿ì Ð?Hl?»Ã!¨FZ­¿âMUô([i¿äy^½zŸ¿ïëÆ!·à¬¿ï"ÝíÜgUNASNone?ï`+ýðíO?–­e{>l?fþh‡Î?[h¹qåc?'¿Õà (?–Pê‹÷
?ï–y$jSÂ?"Ð1Rª¿(?_;,ï©Èõ?eˆÍ<Ó}?†zQC®De?ˆºÊþØÄ?î÷vB–Ad?Œ·"¢F­?"0¥?}Ό$	Ò?˜ušè¢a?‡^;)Ó\?ç¨<Â?~c=
þ-é?rä-÷íx?TgϽÏ?¤›+Åú¢R?|w/oÚÝt?îp¢ÕœC?ž» —-¼?|JËþ?¨?ré¥o?¥vUºáW?'ŒÓå?î±Zk‡~?¢Z|hÕXA?sDþE€N?€ÌÜ¿œª?¢¹Šó? £Âùuˆ~?íɤת?›º?Í#?'……¦Í¨£?‰ÕGúÓ`ß?ª,ì·ü?–CdŸ5¸?ì³LÕè÷?–Þ
Ÿ±¯½?W>¤?núxx*?¸t£à?Ql?•Ó‰¥;ÖsAGN4FGL J1954.5+2420?×:JT3¿ýäH•:À:0S5À;¥Ã<*Rº@Ð3öýwå@L¢À‰Èk?ÓZe¼Tº?äòSÍÝn@à:2*õw@÷l¿›áÈ?ïþ
¡ÿϿ㠝™ÙZ¿ÖÈhûí¿è­µ°P•¿ï÷!ŸŒø¡¿ïë	εÛUNASNone?Öz×w(?Ãzak»öø?¨SaWg?§¤Ûë>K?ã=ȤgÕ?ÄMüjÒº?Õùù¥6ʆ?Ä|ŸãŠ©?ª}ˆÖx©&?£åJÃ\\?ã[* 4	ê?Ä.nï28ž?ߕ%}àLÿ?³L
úÂÄÚ?ÀÜà–M?¦I6:/Ãë?×üj;TŒA?²I‰pË|è?à<E'sÚ?¦ËÚUîÁa?·ÍÝ:è ?"}Ðíª3?ٔP'q$?¨c4×ÈàK?É¢_+ž?¼öCÏɽŠ?ª³[;}?¬FóܝÈ?çì6¥ê›ü?Àdk5>av?ÀÀm÷\öÚ?·U""wl ?¬ÝMe9?«6Ñ7ë~¿?ê}W»ö?º*_˜¢á?Չry3Š?³0ïØÄo?Åu}Óaß?¬nn'Þ ?ß¼FÐbÈ?µL=,Wã?ЏÍ7«½Þ?©ó",<ÙV?¼Ã/nqfŽ?£°¯… /¹?ä³vådž?±!S
£i˜MIXED4FGL J1954.8+2543c?ïÿÒݏ¿ó4(%¸÷À9Q,?#+~À:Ù­´Ù'@
O$«[
@œãÞaIÇ?˧tù|-M?ÖK^£#†@JO‡&ÐN@Õuèºi?ï袠ÿ>?îFâ< š?¿ê¦WþÊ&¿çl1aKõL¿ïñ½m捿á
qs	âØUNASNone1?Ê?íKˆø?¿ëus8u¬?¼°¿ÝÈj	?·è—œÛ?åÙì°ö`"?Ä£"ÐNXö?Éz«ˆÀ"–?Á.´5»t?ÆûgÆIH?¼RòkAí`?ãâ{,Çh?Â
	l	À?Ó]2øS?°²Ni—Ë?Ã1´ð""V?ªœ=9¶?á…ªbÐÁ?²",^
?Ç!Ihv-{? ‹ÉÎõÚ?Ô8ëÑAH?«ò=î¤Ã+?à7½AЖ?«ýf°]?Âyfáq±?¶Ô9ÒA}d?ÁÉ胃úî?¼÷@=ݱ!?æïBf¤Ø?—ö¥Òü«?°ÛÁ›yT?°¢Zž·/?ÍJÖü.Aå?Å,3 Ò"-?æ'Ò
å'?'n4
ft?Å×Lç~Í?§ìWè°i?̔I3áÀ?«Æ(•×_?姴\ñü?±"ò/TM×?®*ôòÇ?'a€VG'?ØÅSUVb|?µÛsï~&?ầzԙ?µvõ‡‰OTHER4FGL J1955.3-5032¿ê&&Ý[ݙÀ>'àãF·À:ÀöÞN«À<r¦Q8ø@bü}"€U@ø½=ã^?¹÷(€|½¿·vœ¿há?þ{ÓJ•Oˆ@>•=im¿ãëÙ7>Z¯¿ä[ÇqC9;¿è"ÏöLø׿䦰~ L¿á¬ïícEJ¿ÊNC"å¢UNASNone?ïÌØÜá©?€î8¬•±ð?CÅcLå?S¤h~"?wåHr?~6rÚn½?ï¢cï,Œë?‹çPXHp¦?Xß#nŸï?oyÞêæÑ ?"KËèÅS?‡Y떭?ïQøç÷]?ˆÄdß­Ä?`Ÿ}©«?aM󻿂?"¬ófà ÷?ˆ;Ê`Ñ?ï°ÌqeÑt?b…¾‹"S?K¹îÌ?4Ê¢ê!—G?'4N?aÐ0ï^	²?ïzytÏÏz?'ð•oaŽp?XÎɅÔB?UûjçH‡?ŽGɌ3Q'?'¿	KË?îË»ù§¦?¬†¿åÆ÷?j––à¤Á{?….M¸Î?¡šÖù	?«ø×îS?á¿?•ˆ-v­G?o®·î+\É?kqppV…m?¤Dûµ'Ÿ?"Ô.¸F¥M?îÔóÛ7&e?…ÓÃû±«x?j‡
r`î?^nh—2?¡Q¡÷û¾?"åçðaAGN4FGL J1955.8-1657?æÀ-ÛþÀ5¨ßXÀ‹vÀ:i1òÁSÀ;õͧ¾‹@+ÌAaŸ,@\…×Dö?Åy£¯ò÷?OÁ—ËŸak?û€©E5?Û&¸{‡	õ?×wEÜ®S¿éDÔ`?ù¿éhšô¬·¿çÉc‹À"?ᐣñâ0UNASNone?îê{²0œÞ?´ÔJ¼)j?i8"8Q?ŒøËáç?Ÿ‰w[­Û?´|ýžg8è?ïrÉù³µ¥?ŽFêÖh¦?lΌfgv?sÒAE
œI?ŒÞlj3?ˆwRæJÛ?í_QŒJã? @…\Cú`?‡RDÔO]?'â ôOÉE?²ï9D€?ž1$•Tž9?íšæEnÊ
?Š	Kt¤?'¢Ù*7f?gҚÝâ'?°Ôz"p*?ˆBQåú?îDÁFöx?°ø—êûˆ?uÔ&¸Çvh?yþ/rW5?©/•‰,?°¬2ÜPl?îzk'3:?¥tjÓ6?3œj‡È?Ž¯Së\?¤‡Ž.ul?¡º¸Õ³¡?êäNÖ[?«Ci5A¹?"ˆ›©ðýú?‰Û t*#‰?ÁݲOjmÔ?©VM/+éG?é"…¦ü\?£üДAí?™/øÚá|K?‡ÒK"Z?ÈOêG ÂG?¢º×Üê4
AGN4FGL J1955.8+1154?ææIˆ_4™À ôuĨ;À;Ž"ÝÀ=óí£*@ "µ$¨?þNÚ"ö¥
?ÛFqÏsÆ?ïn>Â2"þ@߃ê?þ÷öüK@?ÒÖÊ|tW¿ïÿëJw?ïýš)âQ™?Á» <‹v–¿ìÞzt¿ïýSG¥°ÿUNASNone?Ú0û÷mñ[?Í$¨©µy'? ŽTLæì?—Ï€z7?áÞ N¿€´?ÍûÍîWXy?ÙÈZ)õ¥?ÌøډpN?¿¢;Fۏ;?Á9ìúƒƒ?ߨÓEÍ?É'ÚDY¡1?æ±)8Ä©?´*ít¥'ô?®	 Õ¬}?œ§p	ô(?͹k%èÇÕ?³™ý=]"?çߛ"¢o?²Ít¬>?Äц6?±lÒ¥a o?¸ñ"ؐ|?¡µ;pv?ÒÈ4'ú`?Ê—Ùñ¾?«j넓%?¦>O-%,S?äåF­RLî?ÌJQæ3H?ÎH{ތ?Ë~üà:è´?Ǟ¿É.1Â?Éûyæÿ[ž?â†1S(?ÍÉÜò"¶}?âü84Ø?»m´Múß°?²XŽ'þ? ßìL4…?Öiä]•ºð?»‡*¥?ÞÇw5_ç?®?'!ò?Óa†bí?Ƈ䃀[8?Ë­öӆzX?º¾&°æ4MIXED4FGL J1956.6-7011?¯¦ýo×Ô=À>ç¶þ.n¨À;™÷
ø|À=V%Ýà‡@((ú@@«~žk?ÔÄ_`7Î#?ïÿäâBTä@ÜR¾éµ;@("nmØ?ÓڞF§"¿äëgø6Ýã?âËà=ÂÙ¿àhK_·K¿ïÿd†'V?áécÜHkUNASNone?é óÌQ8?ÎÕc|Ú¥?ÅíbPyŒ€?Áæ溚×C?¦;9þ-¶Õ? š¼™ÎÈ¥?æÝÆf£šq?ɪpxÛUs?È5—3[§?Ŭ}òe?¸¦žaØÌ°?±Ól̈́ò?ãÖKz
†?´5°çÄø?Í»ê@>ù)?±
''­±
?ÂêçÙ²R<?§l"¬8»Z?è{
V‰é<?¯‹z&t¤f?dzø¢`	"?­»Në¹?©x™´?—çŒv3?åL#´\Šè?È,+Â{?ÐZ‰B"S+?ÆVÓÎk)ç?´4½W"'?®'N'×Ѳ?Ý-J!È?Ðoc''Ú\?×)A¨ý÷?Ïç(^ª¤?Çi>jsç?¾÷6éÝ:?àðäÚ	Ì?·Üe'ž+8?Ó]E§_*?¶[«kÎç!?Èݱy|?®3+ãtY?Úój¦!;?¾‡oº;ê?Ü~¥¢fqÏ?À^Û^Ox?ÁßoÙí?±5¨ê€£MIXED4FGL J1957.6+1230?ª§£ÂnM[À!_€™"À:ˆ·m¿öûÀ< d©ÍÄD@d'8Ôþ?ÿ'ØÚø	?Ѽ
éÿ
?ÓÄcœ²}Á@ÕÖ¾¾Q@».\^Ñ¿ïß#FV%§?ë[–©û¿ÓN­âü¹ú¿ã¥*&D7g¿âþP§ET¿ïÿýawUNASNone?ìþÛïÓï?ªKŠçÖç£?dŠú]"\?su¶µéi?¶×ÖO´G?¨ú/.âXµ?ë<6-ØD?ºÃèÚ`<?r¿W[›?wâ×R›.?Ây,ˆ§7?º!Îê_Ò?ëÖ[J˜Cr?¤àJ¦Çs?˜Ñ2ÝÙצ?ŽiÂ!´@ö?»Øò}"?¢L4¥½Ù?í+eÁGTö?ˆî†t½†?ˆ,•0ꈾ?e2Ufã¡?³Ÿ?O:¼?†f"5`òÐ?èlžp1Û?ºëPN)·<?'&HžgO>?…-ïó?̽*Âù?¹äh°ÿ¢ô?åeŒH*?Èytdo°?…í"ÀË¼?'¡dé!?ԅ~Zµ"?È9.¬³G?ç"-ªÀ`?°ç¯²Í­?¥¨Íf–0/?"׋TvV?Î
ûr…6?®Òá¹Ãۍ?êQe'«?ž?·uٓ2?'oš£¢
?y¤°Z?̄t³?íðñµ´AGN4FGL J1959.3-6121¿éà[®bºœÀ?¦bfýeÀ;¢™=SHÀ<êI"Çȁ@!VH‹´ÿ|?ò+ŽXó·?ã8b1?í'ѹ›—¡@N»Ÿ}ß)@\ƒÐ`«¿ïÿÓõµú"?ï÷AJM+,¿È=a	…:?æ"Ñá^ª/¿âQ'W«¸€¿áÃÙDr UNASNone?ïÐ͋ʵ,?€f™aBi¢?Q&µžúUî?Wµêw–?sOŒ¹ ¦?~`‰U¢?ï•ê8©¥ç? Õù/!â?hBÞJC]1?¤ìTv
?"tºC®Ù?"=2C&ÎÔ?î@.õÐ?œ²ÖLþ5?…'bPr­?ˆG¬¾™Á"?¦™,ORôP?™dÖ%€4?ï#¶çÄ[?"ZëÛq/Œ?gÉÉ$9û?`€¿·÷6Ý?˜éáhaÕ?"!é‰nó?ï´Ì¼öYÓ?!²lû13?füm»ý—?rÁèƒ9Ã_?z™#/¸‡ú?zRŽýè-e?î·MKÑÿ?¬@‡w¶£s?€Õ¿‰s(è?˜$HÉB_¾? Z{E¢tÕ?¤n"QÌkø?í™íô²€?¡3­©ž?ˆŸ.ÒÅB?‰ûß'ûï?°¯VLñS?ŸTÀ]±?î¾·`Sþ?ž©Ìíϔ?sõBaÕd?}ü8"²«?«•lF áý?žèC—AGN4FGL J1959.9-4605?µ¡öûÇÀ>­ú‡;À;ßúTÅT3À<푮éŒ÷@"Y:-ù8?óxÏÞ±Ò?à´/è%ç?Ù¯Üüð¬?÷Ì_‰ÓRù@}%
«:¿îØúØxÒ?ﳬ ›%¿íç^~:˜'?ÉWw¬	?½ y1Å¿áŸê¶ÂŸLUNASNone?ï'h­"v•?ƒ¢Ý,ç?S%î9vž¹?S"+|:M+?‰ÍÄ:ú?'oµ«W6?ï¾!ä+c0?'ë!
?Pzš_£
?cÂÒYs?|ЇÜs¯?€
¾å?€R±å?"¤6olŽ7?qß<µÃ¾Ø?x0B®Òñ?£9€d Z×?"}JQ´‡ï?vÿT£?qµ'DÉ¢?2­Ã†ÍÆ?,ya—[Åæ?ˆÊlÜ]t¶?pâÇϦµ¦?ïfñ?Œ$Œó8Q?df:·­÷
?dÚШôàM?±«Çî?‰Ÿ%e8jµ?ïP*ÓúNÌ?—½XÄþa?^V…s,?uî¾xnü5?"='H†f?"±¨AÆr?î(.b>
­?™?Û½I"Ö?qQÇ3·è¼?yˁ-Ê$?«Ràõê œ?˜@†?æ$?î܂1—^?¾ÑÅ+¯?@"1ƒVJ?H1Q÷†¼m?¡÷T+mšw?'€Ý¼ÝaAGN4FGL J1959.9+1833?çû›[)‹À¼Pbîâ¡À:|³_=}9À;ç¶jŠ¸U@æ"Ôei@™íeÊ?ÏMò?Ò³×Ùõ@Ëi¥¶Ž?û•P9(j­?ïýà€ˆÑu¿æG¡Ÿw¿á·T*#¿ù¿àÑNÂò®¿ïýZØ®¿ïýl<i<ÚUNASNone?âó¡ëL¿¡?ÈYW-ÓÍ?¼["?Ënæ£É¯r?Òø[ҟ۹?Á›%þ?á6¿L[£??˜ñaa?'RõxD?—_Âûk/t?Ûº\F@ÅÝ?Â"Xn}?ç]ö
k?¯2T¼Êë?¯Ì+ÐÞíE?šŸ!…ñ"?ʕÖ¿-Â?«¤ðº½¬?å"è—A6? ­ø1?³íÉ;…­£?ŽbGP'?Ïõzø¼V?ž±I3Ù?Ù¾ê)1°/?"ÓÅBŽ?»Ä
h[*•?¿ïkZÓ?ßP<·…,?ÃUnqw¼z?ÐÚÎvÐ
?Âï¥n'êš?¨Ž¨0؇c?©MéÑj˜?æ	®={dz?ðc)ðê8?àâé|/üG?³4½Ñ 2i?»™ä')?¢ž‰'k?×yÆĹǦ?²kF‰4L?Ú0!]O?©Òä1ûø?¿ú¾fqgæ?¡ê¿Y¥@t?ÝÑ/<u¸?«5Âvàñ˜MIXED4FGL J2001.5+1611?ÝôÍO‡/gÀñ¾±ìÀ:ÞkZÁíÀ;Շºtµ@ý-Ûö@Æw}åÞí?ÐR—\R'G?ÛS%âØp@(Ëwb?ùqoXþHñ?ãwÁm9Í¿ààM³9ä¿é	(Ó]à†¿ènn¨TG€¿è±òá‰rZ¿ïÿô╋îUNASNone?ä‹Ó[9ë?Ì·"ˆ;+?°í"^'}"?³Tåˆc?Ò¬ô1b?Çþü~Z?âB#'ªÙ?Å4-݈Ý?ªÖ;ÕªR?¤åqÙ=à?Ø!qõ?Ä&™Ûù?東½c	?°\Ôe9â?±fý"u| ?_–»Pá?Îê
wt£
?­VSƒ;²~?å•>T	Ó¥?ŸõòY%Ÿ?¿Î•o"r?•f¨¤¦r?Éü( ï5?˜‰+¡ê, ?ÙQypj‡o?Ë/®¬?¶w‰ÚäÜq?³¾Ñ¤q¸?àˆRÎUÊ?ÊZԝ?ÒK6w#ð?Ɩµ)©,ñ?¿cj¢O ?¼†ƒÛIðÂ?âí÷¥úŒ4?ÉC™ÆÚp?Þ~@iÉê'?³É¾]Dêñ?½Ýï<–çÁ?¤}0/Ý86?Ú
CÅýzÀ?³ì6<BŸ?؁yV3?¦g½€2þ ?͗«ß?¨,H×a?ز÷Ôbm]?§ŸÁ×ÊX‰MIXED4FGL J2001.5-0958?íñ|1ÝP[À4ß«÷jÀ:•GûATÀ<ÝË!Ñâ@QaÒ-ø@â
Üa•F?Ó'½ÝEÁ?ÃU´'Œ¶?òÖ0=µm5?ù(ï7…Ó?ïšúAп睨ÇßÓ¿ëý7Þ¾'Ì¿åÚKäÚá¿ëY*GÒ'?Î}šàkUNASNone?í°0"Šz²?ÅE'"ª†?xÀw®ª#]?"râ'à+Ÿ?°òsèׅ¾?Ä©Ø:-J?ï"Ã,B²?˜×€LDõ?Ø9†FÖ?ŽÉjCu¯?'Ӫφlj?K&bKÜ?쨈K'N=?¤RVÁgE?"Yæ\]&‹?Œ¹&ʧ:?µåDŒiõ?¢OBò
¼?íPþ¨Å?Iœ¤?˜±Ñ$Ƀ¯?xIX¾þó?°ÙÀ=˜?‡shòE?ìÛ²G²¾{?ºsù%_#ì?‰šiùY?‹2'¾s´&?µï !J?¹Lœ,²?Í?í.	3–––?³–#Ažfû?Ÿ$ÔL}D?§%ë[Š´?­¢'?ªF¡Dó®?ê]"l®!?¯¯eR¨	? W§J üÔ?•lÉλ??Âu ¥I?¬ÍØÊã¼É?è=÷Ooí?¦¤©Ò?¬PÕ¿ìh?—(¶ßMù?ÈN/2s?£²Ž7ZAGN4FGL J2005.8+3357¿Ù«;/ßtM?ñxE܃#6À9VÆÀCQŽÀ:›tkâ§*@ >vx'GÃ@ãÕº²?ÁYɟñ¢o¿¨-;¼2Ž?ð%ôkwG_@ö§uzU‡¿î
9	6	§?ïí֝0'¿çÕ¹€ቿë9ÝaD"ƒ¿èïî:ß?Ŕrþ¥7UNASNone?Ü<MÁ²p?Æ}ÏlAû+?†F˔´²?ˆI7<¾]"?ሽðª¼F?Ǝlk¢L?×
(	çèæ?ÐÙ?}T¥°?"Í4)<	R?£:J§Õ?ãÛY˜ïó?Л€.c•§?ے»ü¸?µU#äYÞ?´Tƒ>R9ø?£JܖE0Ÿ?ßXÒuitÊ?µ÷Ð	q?àû(§ûÇ?°S«¤E?ƒ|‰WEü?j|"P†Œ–?Ýq:Î:¾ ?°:°]Eúb?Öv©î?Ä+A›Å‡£?‰ÿ>¾¼"?…žO™—×}?äˆCJNû?ÄP7·­I?Ó"9z8ïú?Ê¿5EÃ>ë?™8‹îö?¬J-Åw9?å¥#"k?ʓQÂ
ô?ÖbÇOà=?´úJtZY?¶¡ðŠ?¦ Ômó?âÈ5‹R?µå´pt,?ÑC³®Á?²HŽæE?UßÀ?€ëüÒsáÁ?æçñ Ç©U?²oÕ»ËØMIXED4FGL J2006.0-6538¿êôôx"ÃkÀ@ï$©ÁÀ<©1½nÀ=¬tg°é@#'ó‡÷†?÷%ˆ»%œ?â}Ÿ"Ò?Êb¯ã Ü?îÓ·¢™œ?ô qÇîk®¿ïZu%F¿ïö†5•8?ð¿Ó½SG¥°ÿ¿åËJÍǟ?Ðmû½ñhUNASNone?ï±aȃ"?•Kòþ¬ò&?E*ÔTÉ	?U)\ƒ?ŽÀúV~Ùþ?•Í´Lz?ïMÇÍDÒÿ?—k
·bÖ?p"lý~9?|éÙ´z
=?'>kdЖ?'
Û?íveþ?>7?¢¦È=\\?v/!¯hêû?€Lu[B7?²éÝòT"Ù?¢XRØH±?ìH1g ? è"ŒŒØÐ?dIbW·™®?ZOs™Iy†?¾ƒsg€Â³? È©Þ¯ö?ïBSáöÌó?•c.Ð,eª?Q–¾X?`:襱Â?–£ªSK¶?•<$ívñ?íþ{0"»?´2˳‹÷ß?}µ@•yªã?Œé¿Ä??¬a¤í'p?²ï±¦.<#?íz*֘R? }ÖDš¹ª?sæ‰U¹xè?}#?NbLE?²ð@¶§½? Ð7«â?æAoeWa€?¸†>RËÿÈ?dÜ«ðé̊?m¤Mè?ÓSgÝ3?¸ŒþQe^AGN4FGL J2006.4-0354?íb‡×­ÚÀ2v…¹èÄzÀ:àUӌÚÀ<'ÅÅqŽ¹@›,™f
@a
;Ã$­?ÉyD$>û?•P?J£?ÏôÔ¾2Ö@þv·Au@?¤–á?æ°§2È¿é¬"qÌ¿æq²à<–3¿ÄïXgö…¿ïóqal+¢UNASNone?îa2	Ï?±tD2èh<?fת²)ã?oò­ð¹?¨Œ°'¨•}?°¯|¿J+"?ïÈ&ƒ]©:?y7‡ê'L"?Jq{taU?VäñžÍ¼à?xžŽø‹)…?v8šÍ·ˆŒ?î K?"3Eý°?uŽªÿ"Ú}?u…ɳ	O?£MÚp§Ç€?'³.œô¸'?ï[_qՅX?r®FqúÔR?W
õ:–?E	"ëšn\?"#±â
Q?râÖ-"'?íý—Å7?©mÙ ?w	EíزŸ?vv)G
!_?­M…ûÊ>½?§†ÿZ‹T?ïsØûaé2?"W4I|®y?\¼8Û^Ð?s ñ¡ŸJÔ?r:ˆ5|?'V·BÞZ?ì£oÓ?¦&Z%Éé?ˆã¸‹G'y?ƒ‰ð¤ƒZ¦?·ÈFˆù?¤ÇŸtü‹"?î#Ы9æ<?'H ‡99?n_:&ZÔ?cæw†ßÙ ?«Ý¢gT•?Äfn}ÀAGN4FGL J2006.4+1834¿'ñ6!œÀýۘAªÅÀ;'~B%>À<Xæk"@ òc'?ýlÖÂïÔ?Öô¢Ô«¾_?Êö²¤W±?ùŽ"î9.@–Ѿ#<¿à O–@I?ïñQçS`пíî+÷Տ?ã_ïSàR¿äËôï#¿ç×Fm¢šÊUNASNone?íEE!¥Ê³?¯¹°¿"Ä·?d‡ôZwF;?nKîж›ó?µ1—O-ø?¯dã;ã?ì{ƺ,•?À܄#0?VMÙ	˜›r?p4‹ÒûrÏ?»È˜ywÔè?¿Á]ÃT¨ú?ì£KR0F?£â|{?€?z™4MFP?y(¡é°?¹EDÆ´¬?¢¥Lóòß?ï^!(æö?|³PTIÄ?aç³@©OZ?TT#æ]›R?'%rvI?{¶<[‡²?ëÁÖº?·Å©`u±?~§¿s?"䀵¬{?Àl—¿
(?·$|¾Åâž?çh
s	H?Ê35<€—?i¡xÑô*?ŠŽ8"¯;g?Ðü¨×˜?ÉÜRL5ú?éðrµ:p%?ªOâ}§å?‰Â°-´5?…®2F½îQ?Æ¢
'1ƒl?©}8s¥½?î_íÉF°i?˜cÕ<‡ð¥?w°Ü_ž—v?yM íÿÙ?§ã&À?—
c"n/AGN4FGL J2007.0+0707¿Ü?N ˆ1yÀ*"œ
!¼À:2wKøÀ;ðK+w}@`Õ²yc@YOýnUH?ÉÃ]wÕN§?®¿»ŸÜ\j?å:áqÊ@҉SP_¿å$ô,¿æ6¢ôŒ.w¿äþö€$}Ž¿çiqÛ¯¿àîç©Çå¿ïÿóÖ&ãUNASNone?ïp£¬¬? Ö²:æ‹?WKöñ2
«?Icû¡E‰?vË
"øÎ? Íbª]Ä?ï~@ƒŒ?'ÆKEU?b¨Ä¨?kóyÍ2
²?‹ÅÙÊ~lV?tCïz?î1øܱW?–쎖صh?~°u\-<v?t¯­
ôRˆ?©
cò["?•l?$uX±?íêõ³º›â?"Õu-w´!?iþõ0F®`?O¼çÚÃöR?¯°µr›±?"mwÌ2®?îĉó;ÿé?¡$rïïc?i0VØ©wÒ?^Íòç똉?¢$[_9Zñ? ÅI¹œS?îˆ×Ø!?­ƒ…Ãb7?soeKf?ƒ@£Õ õ?¥OVÊÿþ?¬'6¯ýNÄ?ë´¼~\7 ?¦Ñ–îÀþ½?pW²Â«#?'¿ì|†–?¾>ÿ¤»?¥‹i>عÝ?éûWÏÛÜ?¡ItV?€Á—]«â?o‰?ƒGxˆ?Çå+OO? »ÉÝ=ºAGN4FGL J2007.2-3157¿ï:Ô.ëÐÉÀ=1ðÃLÀ:=ƒá¡pÀ<<Ãþ¬C@+,õVƒÅ@¡|å-ì¢?Äaºö¶€?È´ÃÁ‹P+@¨³Ûd?E?ïuo]þ/?îגŽ¿Â4]ë¿ÝôÑc4'¿¿âŸ……`ý¿é¤IöÄ¿ïâòÞ¯M`UNASNone?íðVÍA<?£ :†Yc?'ŠjzèÁ"?Ž⁊œ?§²ÕXK@|?žÂ†ÈÁ?鞴Ût?Ã[vŠî'ˆ?»×DÔñ4?º¹jYåúp?·3CÊì3+?³Áö£î"?íïvcOç?°S"k?—ÐÖãKT?'üi¼iû?¥ .Yë¿è?"!fêá.?âQ Çda?¥ªžŽEßz?ÅÏR'?ŸX×^U‰?МØ]µµ?¡Z'ù4?êû6N	'?´¯Õ÷í?®'²ž	?¨îE¿
,Ê?¹ŽZ ]?¬1k'VP°?ã[Ôݬ2?Ìj)» Ž&?Ê2­‰2¿?Æ]L–)'?Èa#W?y?ÀÚ=:jv?ì&¨;·«?¦
2ãöí¯?¦Ê'ÝXMX?›Ï#—`?³iáÏä|?³-AB±?Ôض…7·Ò?¨Ê©DÓÛ?ÏWւÐvÈ?«3"őj?Û{^9`Ê?­ÓbÔ3MIXED4FGL J2007.9+2511?ÛÙÁ¹PøÀÌ W"ýÀ:Vã®À;Úà!p"@ŒÛâêE"@Â&ޑo?Ëk›¦ÿ?áqðþZcy@•ÚÈ8?ìÙAéj£s?ïÿs}¦¿Ñ¥!øxLB¿š…}`††¿ä'á4¸Ä¿ë=3g5™?¿ëëԚ ¨UNASNone?¼ÿÚÖ6?ÁPä>È,?Â#%¶•JL?¾|ñ‡1?ç×Uvÿæ«?Æd
‡ÏË?Æfüìعs?ÃåT-(Ø?ș¤Hý?ÂݹVM?ä?ÿ[·®$?ÂF¤ÎšÇ?ښFS\¯•?²9¦/
Kâ?ÊB÷݂ä?­iHʇu?ØW1Ço¸?±V%QYH?¶ÈډÂij?cªŠ²¿é?à¹Í¹m—?®œÜ5ž¾	?ØÚ.;Éý?­Q
PÇ?»û0*Àù?Èÿk|ó(?ÉíÔU':?ÄyÕ{iz9?æ$åg£R?Ì
L,1ý?­OSÛ§å?²û%ó×'?Ì­ùYêúW?ǙQÀXB?æÿÄG†ì?Æ¢_y?å|?ФIÉ«7Ú?®M¦LÁŠà?сϽ0çB?³Ñ7:øÑ?ÝÙæz6Á¢?´|Öæ?–YǗ¯?z·I·íz?âv\ÏJÖ?µ³ÅÎ].?Ù©pÏÿdØ?µA`0b
œMIXED4FGL J2008.4+1619?ïÛð3â¹&À!§"š|©À:ÐI!²oÀ<Aٌίü@ {3§ø,?Ñô{<ŒMV?âÛ ö¼Š?ïÝÊì!üª?ûº£º"ˬ@¨[#*¿Ý]pH'¿ì9)í9Sß¿æîá(úJ?µîÓTPd¿áÆsxŠ¿ïÿþøþ"UNASNone?êÀwË#æu?¾øä ª?pdeuɲp?j [¢-?Äzý¦x>?½­€"Çw›?ê~µ¤Uùö?Æ~™©E?e87'®í?vsÁµ˜Ûà?Å°I//(É?Æ?ÎAl?ë«:xÌÅk?§!" ò?•ÅÒ`H¡?%–+iÔõ?½4·¤"êû?¥°Hí
®%?íE°øŸ¨@?¨ nÛ?KNMæjl?NÉ	ZÓÏ?µ›Ûõô¹?¨!ðô'g?æü»Ð%Fá?Æ>Çì?|çÒÎJэ?|>†\R̹?ђé´Ö?Æ"*ŒÆws?äpsæµ3Ý?Ï­·x>ð?zUî*áÇ?–yÛÒèßl?Ö¶öÛ­Ôÿ?Ï
@å×?çõ¬y	?°5OVb3è? ª¸[îÁ©?•Ž¨¼Ü› ?Ëþ –œ?®È)°¿²?ì&'o÷?¶ã¿Ž"½?@ê‹OËG?Qhï]ëv?¾©?SýÙ	?¶çͼq—AGN4FGL J2009.5+2425?é1«òjHÒÀïdþ‡YüÀ:Šh¤.HÀ;hFDe@cÉÑÅ°@§ÛðuI?Òò)=;å?ÜA^#÷«ô@äàTi
á?Üϧº'i?ïþr–öQ+¿×æÓs¯û¿ç=¥b$¸F¿ìŽpK™\¿ïÿ']<9¿í·ØIёUNASNone	?ß%`¯Ã?Ï¿"ÜV¾º?·Q§]>¯?Ä#'³#â?Û;Æ5•q?Ï6ú×÷?ÌQÉÃ¥?Ès¹1?ÌqXVrb?ƳÒÕÐVš?áÞæUñ	~?ÅC†½sé\?Ý܃0?³"Vˆ©°‰?µÿâ5Û'?žØ9áyâW?Üß¼×>ô:?³"n¢œŽ?ªYær²œl?…À‰E?á"m~]©?­œ¶gC?َ†V¬ñ ?«ˆ÷‡vÜt?×ߊ'X?Ìك°_j?Â2ÌþB]?ÄÁƒçk?ßÿ™ ?Í&xËÔæ]?³£HÍïϖ?ºCFރ%?ҍgøj?ÌkÓçâìŽ?äÐW›ÈH?Êâ5MÙk…?Ðþ ˆFò?±T8~†?¿Ö²29?¥<•?ã4ùÜÐP?²øÙØy‰?‰êUJ"‹®?p›.F½¾?â¨JâQn?·MH@ã)m?Û#\À9/e?¶é—§sMIXED4FGL J2009.9-2116¿é#
"1œõÀ:ZA€ÓÏöÀ;	±oy4ŸÀ<ÎÛÈRé@àµFsW?ý…Á•a&?ÎMúI\ÀJ?ãÃBàO`@´Õ½6VÔ?üæÒâ¿ï'¡­º8?ïþo§WÈ>?Õ-•d€³¿ãb:[€Y¿êÇ
H½ß¿ïÿ²2ӁUNASNone3FGL J2010.0-2120?äå >™¨?Ĥ:ÇÒ/?ÑÚ[æ°£¡?Ã?¾Jµ¶?±mŽrÐÖ<?¥¶¹KKéõ?ãﰚš©?ÈÜg·Í¿?Зó¡Íś?Å£†ˆÖäå?¾"¬£ó Ý?²ƒÃÛ(ޅ?â³û%v…?´âVvl3~?Òóêæñı?²ÿKw"-›?¾{<%9?¦Åxsõv?åòe–Ãâ?¦¼
Fh?Ç ÒÍ0¹ ?¤æ‹&?À•–׿¼e?ša¦*z¸?Þìðûø€Ò?Äeà&ZÃ?Úâ•O̵À?Äꋼ-º›?¸ÁæÏ¡K;?ª¡	¹1ýc?ܼ¸•»Ç?ËÿˆÖþ©ê?×Àj°ÅQ¦?Ëëq"û¢?Çï/o¦£?»}=›ZÔ?ÜùËÝRoÓ?ºf>x`º?Ùè0ŸÀG?¹"
Äè?Â<ŸÌ?©²'ˆnÉÃ?Þ¯ø‡!??²×Áe.'?ђ';âŒÛ?´÷Î1•"?Ï{
wÓ N?­	xåàAGN4FGL J2012.1-5234?í£Þjð À@£}é9êÝÀ;CšMô€À<¢È£r`p@"¨YßDs¢?üé
	Ó¾Y?¸éú=|b¿ÀJNØ«'a@ñÿ ÜïZ?òà-"ã§Z¿êiU./¾4¿ãºßr#¿ìyÄaÄ@6?ÞpØûYR,¿é,Žž"Ô^?Ð;e[Ï_UNASNone?îоä#M?´¹f=¡¡?T[Õ¶ÑÉ?aÒA	ñT›?¢SþÞ+"º?´YǂY7ß?ï»tQ?ªH Ü¾D?":¢€z9?¤ª»ÑŽ
Û?"ˆ©š3A?•|n'Âý?훲KtÑ?¡>n÷?Î2?vë6êyè?VpJNŒ?±³´³1o? Ÿw‹õ
«?ìäáà ?¤7´¿hJ?Ž©û?"Ó³ÕEq?µ
0_J;®?¢´Í`GGÐ?‰˜3'?®/ÃOìž?ntSLJáÇ?s¸$qhëÙ?¤ï"5«Á?­+%¢ÅÊ÷?ìڛR½xW?ÀQ^Ñ`t#? À>¡ŠÛ?µ­2÷¥Èº?°Ë*¶}?³eÞš¸<?ìã!ÍQ¤Z?¤T¢q>©?|ÞM҇?'È´ùj9X?·¹ž](?£Ñ‰¨"e+?åÏâӖ·ß?½rsdý?°"Þj#ÍI?¬¬е
?Ð?¾eÏ?»cÍ;ÔäÁAGN4FGL J2013.9-8717¿ÞS6'}	…À<°_®¼À;¤'[rÏÀ<֑¹ÑG†@!29OWB?÷4Œê^®?Ù=œ˜§?Ø}jŽê/?þw'Þ"um?úàï""n¿ïýxÑ¢õc¿ÝñïÜqZ‹?ì÷ª%Øם?²<£Ip·M¿×6‹{U6¿èŽá¯²áUNASNone?﷌Ù99)?t»MšNâ?Ejœ:Ò×?<0výyÉ?€ÆèµW?sÔáÇBb¾?ï	¹ùFº?…pÍòUŒ?\"}"ù}Ó?f¿Ô>Ϫ=?…-ê¯Ò?f¦f×[Ž?ïpÕ!§g?ŒÑB%µo?r¶²)²?u'mÅdÕ?˜Í·¿…¢¨?‰ž>ôüN—?î{í]Ѷ?‰·Û}ww?WÅØ֊)©?EͿȀŠM?§'ûcâHL?‰‹Ú¦Ä?ïlž¼n/Þ?‡Ø.£¦Ô?Sì{…Ïá?N³$¹Ï?'-`¶N0:?‡Ê
2v(?îøzŒQ÷2?Ÿþ+¢?k?èãÚ¶•?xÓ\™h±?ˆ±ZyŸÞ?š	¬u@(L?îqâo?–ꐧä}F?u¾¶Ñ¼4t?{&e½®?¦79%†9z?•[£Œƒÿ?ì§ô'ÛÜ­?£5Ö¸«M?^î«åc«þ?\-ÕA5¸r?ºD »CYé?£4/†¦-ïAGN4FGL J2014.9+1225¿ë»rkúœ`À(n$ÛÀ:¬%¦'¶(À<rÛ¿®×@'}‹qÞ@|Zœ-Ȑ?É¥>}êª?¨ÙMþTs?àá¡Au@Uzæ{¯¿îxx¢(3{?³/ÈðtFÏ¿ë[iw'ß¿Ï*ö´Ò°¿ãê–vÏj6¿ðUNASNone?ï·ôß¡¡â?y7'#"vz?Q¶©ÿQ11?NÎdz?—嬛»?w–+ڈ$?ï¬èa¹êƒ?‰U։)­û?Gø·_Ò©0?Tóó[ݙ?ƒF\"Bg?ˆ•èŠ›}?E;É?'EN'{%?{±¬·Þ@?xa¦°•?¢'©b!?îîn´2?ï>gŠ¹é?vÐ+®.þý?`‹ZÿÏ´?Dõ꘻†/?–!¬%¡õë?uÑ)º£ÔU?ïK˜­w?	¦xÎh›?h¸X&Â?bà0A:VÄ?"yö.­Ù?÷µ/ŠË?îÚkØLˆ?­E¼û-T?`öˆAáV‡?wB=º
>?¡IçNµ?¬ïÎ78®ü?ìúª‰3£?¥("¸ÉÑ?Ž"Ý|…R3?†Óž
?·=Žýo"?£ò*C9T?íë9!3×H?'å#…Áš?x9qðA?f+vÂÔL?®Ll%~Oø?'AIÝޙAGN4FGL J2015.3+0758?ïmœQÀ-:}ªOÊCÀ:hꭈcçÀ;ÙRé±ßá@…xÐK\u@üô}þ•?¿å[9ºH¿²Ûae¿c?ów¨Èá…Á?ü³…ü-ãh?éà"¾ŽE©¿êûêâa‰ˆ¿å2d×.¿ê÷Ü_ïT¿ïò³±rÔ3?ïҌ)nŽSUNASNone?ïT²¾:Ÿ?""Ýïl±o?e>]QŽ?`ŽœvQðª?'ǶžžLm?"QÀIÙ(U?ï9GÚ¬? dj~
?vdöõ`w?'1Ñ`ù?"F9A·|Ñ?‰ÊùËÏ?ìvˆ9—GÒ?£ù;Õ>ƒ?•š›-_¸?yÿœï?¶ågìm?¢Uâ&ÿ‡Û?íNY¤á÷+?"¶£ô"?…ÚœÝàŠ3?qÜðü—ï?²Ñß=45^?'ªófȳ?íð™*Û?­G^øËé?ƒ>€ñ8†>?6DË®	?¬&Ï´Ÿ¸?¬¬KI–?íÅêI×±Ð?µyìwtÒ?'0ô*p?žÒVËÿøg?«áQÉ^I?²Uª_©?êd4jã?ªü¯ìÖÓ? 7®ÈùÛ-?"B6»ÕÊ?Âa›{q?§ÿ.|rÊÖ?綖Õøx*?°J»»ž;? '%®—*õ?'@mÞsËü?Í=AÚ?­Z
OXzAGN4FGL J2017.3+3525¿Ê&ÈÅðÔX¿´u"–ØÊÀ:Ç>A".ÎÀ<)I`œ"@!½Hö>
?ò_æ¤ì´?Øu\"•¬?ïÿïÚê@
É?äò]€?ü(^Η}5¿ëÖ?rÖÚ¿ì| ·Ûy¿Ò]
øGv?Ëz£_@,k¿åê{3}¿ïÿ~?ËòÝUNASNone?åNž"ç>y?ÃkKT´"¤?¯G4Gà][?­^Ú%é«?ÑyÜMPôB?ÁµÌÈ^î?Î,h&7ªÅ?Ê|–¥.´Z?¨Ô6¨§ŒH?¬Hd)"…?æ碋°¢Ë?Êll-u.?èYx0,1?°`ªÑڐ ?³º+/dº?¡ÈnîE#"?Æl=
LŠ?«{(uK#?܎"/é¨?´­¤Þœ-?°•‡:ä†?£pòi;_?ßL#îácw?¶Ç˜RÄ3{?Þ«Û_=?Ær#ŒÖ?¸óâql?µµ,ƒ¿Þ??ÛNã+ͨ?Åú,'6‹é?¼™•Eš?Àª/¸n4Ö?°Ü·ùÇzÕ?ºž–÷†gk?êc•ÍËê?Ä-i£:_Ö?ãÓrî´þû?²RöÀ7Ô]?¹	ÒNšV?¦8ç÷ýPn?ÒØ-AñV?±.‡2"ïï?ͱ¿Ÿ?¶Õä¦xÉ?µºkìb>d?³ƒÇY_0¬?åÜBžé˜=?¿:Y‹?AgMIXED4FGL J2017.9-0114¿Ø#8¡(¦ŠÀ3¼î9.÷À;öÜjςÀ<[ƒ°úo@ræ@fU@
%ó¯?ÓsŽ!ì8ù?àèS¦pA±@ÚcÞÌ©'@§æž!ê¿ë>L×I''?î‡óÿÁ–¹¿×ó{B¤,¿èš† @¿ïüð§12¿ðUNASNone?ï
$`
? w{4õBF?"ƒ°c?žû¡
…?†rÏ£Œz?°ýðL%?ì§Ý5"{;?³âÕÿÊu?­/F‰d2Ô?­@¿æCó?¨RæçÎq?£ì—_°ÿ7?ìXuë?e?¤r ȁÌ?¨a¿½¹—7?˜óù'ò?±wa[E¾?A²L?è¼[W‹úl? |(J›Š?¼žP",O¿?•Åš¾¹Ü?½~Õ!sÜà?·Ñ'M]?í"OBæã?¬?]Ê÷º«?ªÛø¦ÔÇk?§JAýÝX9?™¾&R
u
?•Ãs‡·?çO®€¨ÔB?ÆGïéï?Å$ôÙv?Ã0ÐÂП•?»8£éqè?´ŒŠkÃr?éH#À›Þ?°ÊýŸ7?¶Qk§ÙR?£ÄxÁ½?¿mû8Ά>?¨¤#§£=I?ߕÙ[%•'?¯X8³ø+?ÎcOgû?­ÌFkÔwW?Ñ8$š¶r?²ÿ×0ëëAGN4FGL J2018.0+7903?׏ݠ&@6©˜áõ²À;É+ml%À=Kh;R¼e@þµFÉ= @lñ<îØ?Õ×Ä3êé?ï&p­F@P¨>x
Ô@p£V0ä?Ô_2€ó¿×dŸg™¿¯Ó.±Í¿èélÀ"{¿ïÿàöO}¿ïþ€Ǒ$UNASNone?ëÔ7{R—ä?½ÈhÏwL?°€áànåó?°úþG‡í¹?°ÝbEØAï?±•… ®ÚË?âÀûÃãÍ£?Ìo®S²Q?ÔI^.o»5?Ê£"—‹?¸Ò©)¶[?¯Ü…Î÷Ïy?éØÖ ,¨!?¬V&)Ý?¸­
>××?£¸c%—¨Î?¹0ò7Î?¡¦È\H×ê?ä*Šî+¹?¯Ÿ¿QÓÌ	?Ô`($Èr†?¬˜Ž†ÿX?ªVüÙL:?˜'Ÿ2xÅ?èEÓùýÄ?Àî§8Ï»{?Áirô>V?¹2*XDïÜ?ºÿBbG•7?²Á·ã¿?׉»;f?ЋÍlô?à5ñÜ£?Ñwr±?Áªý(N¨?¶ô`ëi^?æ@…?³è©êM%?Ã0ò,>´?¬S¨ªŠ?ÃΓ¿mœC?¨Î†e~AÌ?ÓK،:?³íNñxå?âÕâ˚PV?¶8Iã!C?¼$ڌËLg?«Þåæ3xMIXED4FGL J2019.6+0616?ÙݎbÑ'óÀ0cÛ]‰HÀ:žcʪ³À;Ûxâií@ã`"jZ½@8ââ¸Ç\?η:ë
€?¿@1ôCß?óµý˜F³C@Ún9™~¿^£úF?ïõŸI[ê¿æ"@ ×f¿ê}ó¶E¡Ë¿æª§=Ç
ì¿Ê£]½ _UNASNone?Ͽñ?€´ß"+;¢?U€PÁ½:æ?N°ÔK^'z?‡å'JÎr?ÎÔ;d…À?ïpU ùèÂ?"ª®øx
?nþmÏStM?zRßNÆ=è?Œ*ü>:´m?C	Žó"?íˆ=-ÝÞÃ?žÍ¬½8?†ű–Â?µ'Ü<?°úýÚaÑ?›½_Ñ´®—?ìè1´ê±?‰ÿ6›6l?…ëN©ÊJ?jÆô]Ã&?¶ƒ?,?³ÿün?îð.s'ae?"
+B"ý?q§ÆØt©?j.4]5(l?J%î2?'Á\p=Ñ?îe^ß¼ò?ª—ão,?‡NLA¶©?–Úhºçc?£Ö~òf4?¥{Žš Íâ?êÁá•öe¼?©èEÓb¬â?—p±´f¦?Œ¿æK%?Â'õ<?§üõ)Oi&?çȔOǂO?¦3úÄ«?˜ó `­Ô?‰¼ÿ7Hº±?Í¿J´•Yª?¦u@DýAGN4FGL J2021.9+3609?éʎaµ°¿Û5L½j¯À;hÙÞ-GÀ<
Ž7eÇÛ@$‰ç˜ã?éà§_ªài?âÛþCx?ïÿH è@uúX S?üJÓlN2¿ïûš?±Æ·?îJùÞ}Ï9¿ÕÒ½<64¿ïú²]à°Ú?ïåe¶™…?Âw´ÂiòbUNASNone?ÛÞNŠ&´ö?ÐJ[ì?'ã±K'+‰?Š¸ü£c¤?áÅIö³Ÿ?Ð.sŠ*)¹?¾×é$` k?Ŏ$[:J?™¡³g¢°×?¨Qä°5–?ëWõ@D¤Ü?ÅÀ§MióÂ?æ¿8­W?°ºàŽÿ{?°ÿôžKP?Ÿ±ïoǵ¢?ρ¶ÿ{?®Ýzö¿…)?Ú'ö–AAá?À«Í^ÿ%?y—Ð4à+?´Eý?â¸Öy…
W?À›¶/ワ?Ø!A›MEP?ËáHßÎ:?¥‰
˾±‹?¨6¯W…Å?â–ÎU¸ï?Ì:éF;^â?³È÷r^?¼qÊn^é?™˜ËÕ¨M?¬ºá'äB?ìº8¥Zdr?¾"ÆÏea?ã7pÛs?²6âëC?µ³ ]C'*?£aÅËYbÐ?Ô$7æ(ñï?°ÅPÌÌ!?Ä<›¤Ì(?»œ"m,J®?|À ƒÇ\?"sÑiª?ê·Wùã¯?¼5Òõ°ÇMIXED4FGL J2023.3-1947?áè€X;;§À<ÅAÈ!laÀ:Gû'½À<:»9&';@YžP7¥ß@óõÞ>Y?ÅI©Äå?Ä1s*.$?ûL¹ìö8?üþS¶‹¿ÜÅ3ü0耿åóû_‡O¿æ"f"?=¿ç>¸Ø#B$¿ïÿ*LÚ¤&¿êá'V¯UNASNone?ï	㮐¢?²>²{z?€ow?PE?"'Æ.Ó(?–^§§ºžÁ?®y<³¸Ê?îžßی?›ûZk`•?Š÷izåEâ?Šÿ)ºeKq?ž¨OÔyu?'Ã(À/ÞÕ?X'Åd?"Î4é²/?"£þI
)?€š+1S?¡:ãÚ6?'FÏ?í¶Ýg­@ô?†ý«V¬ö?™™Ê°¬Ÿu?xê×›³Ö?§ÅD,Õ¡?€ÆD'b:?îä^9?¡¾W¤b½"?'qFJYmï?‰D"'é?§'ªÕ—|?"	Þ1@?ëÊÐ,l‰Z?¸]'ž8öÓ?¡$Õ ¦–<?£»aí´?¹ËÚv"?´Â›p‰Tþ?íX3kDû?  `2DË·?"Õ/—©F¹?ŒrlñÖ!?°	—T?™ÿdÿ§ù*?êI'÷&ù¥?¢|Õº×?¯W!™À¡i?•}pøoü?¾W|銞?š"p[aïAGN4FGL J2024.2+3616?î¦Ánä~¿ç¿û}º@À9¼L¼ƒ©À:ÊèïBB›@ ¸dÁÅ@XÕ[ç‡c?Ð5†?º•òpw¿?ï¨E™gD³@
,€ÛÞ¿ïù}Ðwl?ïþR€ÖT5¿âß̃ѱ8¿ãV¶Zš€I¿éÆyÌt¸9¿àEa3 ¿UNASNone?Óï´)# '?Åûœ‡Ï\?›)€£\?™S~N±á0?å.Ý?®
;?ÅÆ­Áø;?Ñ^›Ìá?ɝb=YI?"ò)•µj?›ãqrì®*?æ±a±ö²¤?Èë9Òè"q?Öñ¦[Õ?µ99ž¼?µÓáŽÜÄj?¢ÃÄ033?áÌ° yæ)?´À΢©?Þï6•?ªt=(O`ƒ?—ILp‡?|Ã-¸ß'î?à=öf5á?ªA^Á—¿™?Çù3ýn¼?ºô_;ˆ?©…¢,?m?§á7ƒsR?èidгÁ?¿âã¸÷ƒ?ÅlY€¶?À¥µ#ìK÷?š§K²%Ě?¨ð®9Ÿð?éå*ŒEž?Á³´«vn?˞ÕҞ·ª?®y¦±›s-?¹;pv¦¸?¦Kú9Îu?åðÜ|uÏî?²h/YØæ?ÍÀÕó'?ª³ó+%¸?ŸÁ²zV¬a?Ž2¶2å?çºk<JDX?«R»ŠkdŽOTHER4FGL J2026.0+4718¿ì8H^¯Û@^ÂRˆÀ:Ót«£‡YÀ<n´Ý¾V@ø²m¥õÈ?ÿ-5Ã0kÙ?Ӄ_èÈ×?æZË]a'@WgZ',–@²³HÂ;¤¿ïÿÒH6Ðw?ïìrº1¿–¿¥äká
؇¿ÒHSUèiá¿î1"áHÚº¿ïÕFƒrèUNASNone3FGL J2026.4+4709?â$Ož+'?ÅâÛ	¯õ?Á›ÚD7E?¶Gî­Òs›?ÓEés¡Y?Ѥ$.è?Õªßù5?ŔYš6]Æ?Ë7é	ˆ-Ð?ÁÀÉ|häÎ?Ý[`›B³{?ÃÒpdÞÁ?çûý¦Ö»[?¯×¤.¯?¶Ñ´ A?¢
jý?ħ/W9*w?©ÓŸÝ×?æš"Q…ü?£LSž@P?ÃþØËç'J? \Obóþ?Á˜ªªÒÀÆ?˜­""RÓz?Ý_±ôC"?Æ&çÉ0Ë?ÅÑë'øöÕ?¸VηSUø?×·X®As?Äâ…Â]nV?ǎhÌO×â?Â@ aIq
?ÑF¢
—©?ÇF£Ûð^Ö?áyVû[ÍÓ?ȬZL$Ø?ã4²¼Ö4«?µÚóxû?ÀöØu2Ã?¨žÊ¸£ß"?ы‹?³ÙNztUá?ÞÇGÌ6=Ã?²'"-W?ÐÄw:–vF?´[6CŸAB?Ðt@ø k8?¬â.oëOŽMIXED4FGL J2026.3+1431?çö|'fŽÀ*ãjËGÀ:ËSïk]FÀ<«[ï@ôÙ4ª,?ú•çéóN?Ïȅ?o'?â=>»&²@‰`ÈW?þ§^3$k¿ï쾤ëÝ3?ï{ÆKç_¿·¾t¶¿×»o! ä'¿ëko"óh¿ïþÉA‰UNASNone3FGL J2026.3+1430?å5cº˜z?Ä[D}!®?ÒH5€a܋?ÛÆb­ý²?ªhZN\?¦´£
Ë??çݶYmÚy?ƨ'77µà?Æmò¿Ù'?ăý®Ÿ™?´6g´ÞÞ6?±hÜ2À;?à0û1¨Þ?µ¤æÊfûi?ØZ4ѐMb?µq~F©ô?½4à1ƒ†?¥U%Tù?è§N­&7?=ÝäªÂ"?ÀêhS·ž?˜Íï/ÏÛ³?¸ðiÆ(?*×DÁ?ár€aJƒî?Äï׶,CÍ?Ø(i[
lÐ?Äô
MЇ?³ÊWŠRO?¥­s'µ)?àƒdª'(?Ï^#»ŠÉâ?Ößh(fH?Ïg^hÁ	 ?À4ò‰ðÒ?¹³:°Íú?׼ꞑGˆ?·çö<Hn?ßúaí¨1?ºmÏïË?À'fågMl?ª"¦/?ãí¦4˜Ê"?¬É¦níˆ)?ȝ¿…ý?«p!Ú~â?Ǭ`nˆQ{?¢æ¬%p#•MIXED4FGL J2027.0+2811?ÈÏ<>À‡oó­â&À9¬ŠS«x¿À<©"àß@Ans{!ß@z*ž9;‹?Á *†<ð?ë7ZU¶ì@!ýAØèd@YøŠ•Æ?ïû/²?¶Âa C?¿Ü7e\{+¿íô×x!yÍ¿ï÷M@ÝÁ¿ïÎ߁Z]šUNASNone3FGL J2026.8+2813?µh\œajÁ?¹2­éaø?ç¹&=g¥½?È2/+€{)?Æg8¼g­l?†á‡;k?›gУåێ?¢Io{V?çpæ%Ó%?À S`éé'?ÎÏmTÛé9?¿‡¼Uÿ?Çñ'J×ø?®âßóqÜ?å^R›$Öq?³'Bג?•ŽIPÎF?¨ÇŽ`¡?¯JÍLj:-?wó£ïá?ënïâP—?¡7NsFç?´ãmKƒ?›åŒ‡XŒ?°U;‹e\"?³Hz—ì]?é®^w¯?ÅÌ aßÃõ?ÃZ¨À܇3?Áfl}ŠM?Š¼Ðä8ÿ?'ØŸœp—?è[¶Í1 ´?çÔ^«K?ÌåW»±O!?Ä+ë‰Y
@?Àµ®>'"*?«S	.«MÇ?çReÄÇ´?³ ?î0?½pŸ‹‡?ª¹-™Ò`?‡LF†up2?qëtÒȌ?íUÓÑο@?¡`Ü´'p?²gØ¢s%õ? °üÈÏ"PSR4FGL J2029.1-3050?îìÜ`yÏÀ@­
A1"¸À:¬\qðÞ$À<6.#)@"Pðˆi@P9Ô7$?Ñ9¾½•wK?ÊûW2'?õ¬8Ï
@öåS+v%¿¸K"@'ý¿æâCÏb©¿éÍÕáH"Ô¿ätáÙú2¿ïÿŠ#ÚМ?¦¡€Ã´ËUNASNone?ïÍ*¦Ø؅?r1\;èªù?bøðRt'?aqFdÎkÊ?p\0ë#x?fÒgmÛÑQ?YÎ(?…¹#=?þ'?d"m\97?nUÊǗäM?‡—6–S¹Ç?€ù	Ì
?ï$$b
G?… òñ}?y	RäÿH ?uÆ*Ëøh?•9Êö?†oxZ?ïŽæGr/r?jgO²JŒ?b©`Ú]ö?Edw³ž³?‡¿ƒÁž£ø?gÚ» Ÿ¬1?ï˜Ð¾?ÍðÉaI?oËäÜÄTÄ?gE¢¸-ƒÉ?'
'ä}E?{'ÏÀT"à?î¬êëñ«?¡	Ÿ?d³£?wËör"p[?…ª…4dã?¢FR¤|Ä?œŒ$5öNT?î©Ž»?˜ïÈÄèB?Œ£º·?ŠŽC;\¹?¦oeaî?"åÎckX?î½ÐÈ&lH?ˆñ1¡†Ï?v;þ;5\m?bö†é˜|e?¡[s¶^Šö?‡
"r®
AGN4FGL J2029.4+1013¿ë9ãóÒBÀ0dô¥Xê}À:Œ^×ü«¸À;ï&<ª«:@÷\1X$@Ìa¢—o?Ý$‡¾û¨Ø?ÛjŸ(Ï­?òÓ<7¾³/?ø"ãäës·ˆ¿ê"k'Qտᡚÿöø¿èLewS¿ïúý—oó®?ï€Ú…óUNASNone3FGL J2028.7+1012?ëxM;ž»?¸!zZ+?'Ûiù½ù?‡Äü6sí?ÀýM]«×µ?·zòc°	»?ï(¯³P=Ê? TŸðnê#?{¹m3‡{?ƒêؚn'f?"û®NÁàß?œ<¦'‰0¿?骿)Ý/W?ªï¯—0(?®WGh?"O»'?ÁÏþ'nã?¦3ÄÖó½?êÓ†E ?¨ƒÂ×Pjn?
&wí^?m¢ß[ÏB?âå)²Mg?¨;-7ý'?è?-œ	ON?Á0Í?Œù:'BÐD?´™»'–?Í3µç$‰D?Á\1jll?íE,O
Í?¸ •n30Ñ?–®Ô› ¢û?¥Ué@ Ú?°+±w-t]?´y÷\˜\?æçšD¥É?°\,±Êú?µSÿ¤+'?£7œë©4?É·—4æ‰?«=Úš~?ä´Dór?º…8¯Ê?ƒüög#Em?µÏ¼2¤,?Õ÷Žeøœ"?ºe´Wé~'AGN4FGL J2029.5-4237?ïÞºæ,ÀA¾#ˆÀ:͗ZBÀ=Ð&¡@Ö	³2@®ü*ˆj?ɼÿdύq?ïÿça"¯­@ìYÙ?üŒUc_?ïâTžgߍ?ÏkY?aj¿á矶êy¿ïý6AZ"I¿éނ¬Ã¿íœݰʹUNASNone3FGL J2029.5-4232?ÜC՘š¸?Îå~"é×?ß6dplú?ϚbÙáT¼?²>é¡y?°"½›s¼Ð?ÀŠEã'ñÐ?ÂìÃ|÷û?è•2/ŽI@?ÅDtAN§?ºAâ½=Òb?²™)e6?Ú=~³ȹ?´`+ÿ©ã?ۑ¦Ìï·?´è|Ð$	?Äaµ? ?ªñ¶z˯3?¸XlÐ#H£?Ÿ‰Å¶äö=?ëßfdZiû?£²¨&'Ô9?¡XÀ	?'y±è]›?Özà.\?Ìw€7p?â±½Ò³í?Î
<éë@«?µnñZÜ?³D>ąf?²
	ݟ9?»ãâ"¯!?êgÄZÝ?ÃbD·*?º´ÓSFŽ?µ
è}Y&?Ôc¶Á¦0´?´ áU¾ô?à€&Œ9g]?·O¨æ#ò	?Å7øKÎ"?«væxZß¾?'Ü'Bá'?†–U0Lè«?îV©ØÉ? ²´v(v?¡0NLJM¯?™	Z0rð€PSR4FGL J2030.3-5038¿î?N\ââ–ÀB% …²À;MäSÒÀ<¾ßê¶ÂŸ@!üщÊï}?ú¶_¢ýÆj?È¢{1úy?«s¤i¡?ãè‹9"†@ñðÅûLg¿ïøª*s?ïý`t#"¿Ê;-½þR׿³½Øþ‰]a¿×(¹|ãÖT¿ÝáÉÿ={UNASNone?ïâòVQÎÝ?`-ÑÙØÍ,?)Hi2Zsï?,·}¡7s?ky#)À5Â?_–®Øó5?ïØr	)A?qnC{gï?9®ã%f?DìœßÀã"?rXØך¢­?oØlQ-¸T?ïLžs—?""ƒÌ—Œ"?WNÎßìx0?XfωÁèt?•?J©Ø'?"HûH?)c"<?k­[TNà³?Jç÷"*ó?3&ªÀ†¹?‹­×$zÄÓ?kM>îÆ{^?ï½l
´{?œs+içڂ?DQIÿ—?g(Ÿ³py ?~ÉV7?™˜Ou;Éã?ï€#§W¥â?Ž,4ÊC?J¤¹î–{?\'ðÕQ–?ŽLʂ'û?ŒØ
vI?îÍS;L˜p?.†r—Äz?^X#]ÍB˜?`•Á>?~
?¢8/1ê?Ž›âL:?îɶmmtU?†&"ÓÜít?]Ž!Wí"?PŽˆ+x£?¢x(,JD?…þ€|{Ì`AGN4FGL J2030.5+2235¿Ð;³À#yí9SÞ¤À;8
‡=À<'JŸ`ƒ@!‡'Kœ‹'?ð7`Sý®?àXBaNz?îLYµ@˜Ôw¼@.¶YBç[?ên^ýçKÿ¿ïñÊþ@9?ïþ
a'l)?pu¨ßÄ¿á'ïXèϿⓢt3®ƒUNASNone?ê`R"ç?Á÷˜×–™#?n"5R˜a?h"‡2y?ÆeaÐ÷Ì?ÁåàLc±?䅹ãf_?ÊM-ê7Û}?Š},\œ'…?"Ú|åc."?Ö ¢ÖóÛô?ɗò¬?ëöýõ0;?§Ü¡óXh?…ü!î´ ?'þà(Êӑ?½¶‰òæ?§3þBUS?ê™AýGá?ªÜË"?€(O&îó?pŒÝÈlpº?Æ»^Ë?ªNó©ãò?ç7_¡¿òŽ?ÅBÃÁWÆ?€ó"3¯ô?~Jü›Ñ+?Ñ	¨x8?Å+$õœ"?Üè·+Œ?Íøè°>\î?'Êk}åN?¢…yÄ?Ÿ"?àõlÈ͆(?Ícï¢J?è	ûÖÇï»?³fçøÀ
?'@@†Äî?‹XXL@w?Í°"Cáy?³áßFc?åVæ<p¯Ò?ºï%Å¿ðÏ?~")çˆÑ?'£º'{?Ô×õ5‡Ýk?»?k·€'MIXED4FGL J2032.9-0005?ÞÈ"Îå'À6tÅÉ£MÀ;nãª2À<f©¢%YV@ºãÓNœ@{GA1M?Ĉ\ÛMC¿£¦8ŽfàŠ?ã\g	#•?øÃÆ0{s?ïû<aZ8¿è»¸¨Rš¿ç!Ë+âÜÚ¿àÏπÜ3r¿å¦v î?¸¦g¢0UNASNone?諭sSðÔ?{(eêâÖ?@'{B0?2^¨}Ãÿ?"GŠù°À?z·Ä×ÿ¾Ž?ïr2%R[(?];­EÂ?l°—4NŽ?t(¹Eda?ŒGvw…¼{?Š'±¼Ò¹?ïA1–®‹L?"üR¡bÄ?e³hÜ
5¶?`'èG»w?•#`Q¨×?"<- ©°¡?íüðQ>ê?‡T¹cæ
Î?xhTA¾˜Ú?\á%KÍ^œ?­#ðcï's?†©ÛK¹¾‡?ï8Bé"‡®?ÑނÍga?Qðì•(Áv?Cçpdùæ?—Ø"8e#?›Ì"…È?î‹—'%?¥>uO›d?}Ô!º˜ÍV?‹"£%O?£")ޙՉ?¢@T=ÖÁ?î¢0U!3?'ŠòUÖî?o¦%ì?g·;žò3?£åZ'h ?Ç'ºG?ét^¼xì¦?¤D*Ôә?'3ڝÑÔÍ?€çQšëÀæ?Çè	ºÐN?£ñõª¹AGN4FGL J2035.3+0557?èŠÚöŸóÀÀ3ãêòQÂÀ:Ê°'Úb¸À<#à{Ö:@T­›"*r@͏ãÖÕ?ÄT±2<".¿ªÐû«©?äíò¼@®)Zvå¿ß²køvžÃ¿æ°ÕÀ'U'¿ïÿþˆ0»Š?ïÿÃÏÎ	
¿âgÿyÈC¿ðUNASNone?ﱒƒÈ?Ž5yßj\?g
]4ç"ñ?…Dr§à?{±–ͯ?ƒ…â»Àn?ïèÀ8>à»?H­äÄV,?<ÈCÎò?j†c-å'?c¦¿‡íÝ,?~ˆüj€›¬?íˆ$«tÒ)?£³ÝÄjm?fõlrq?q—'L;Ü?³
Rø_§?£Œl±ðWµ?ïðßg?e'?TÓ¾MîùZ?!Ø\"g?!g¤)	³?\/°L™?TXEsH?ïR°?è?"°8ON]5?ræÿ¸f'?ÓNÑ]?~o¨Pÿ?†QÂØä?ï±\f]W?|X9S¾?UÀœ2ë*¬?~ö"gç?€ðÒÝ%i*?š7ΎÈú?íÏ̱t?¤"øDÎ$á?sÏI»ŽÍ?w,³¸	ä^?¶dŒþàÙ?£¾çš¤¼?ïÊGÛ?xO€ÓÈg)?TÝjË;›?f"‰¦22p?u¼6
\?u›tƒi:YAGN4FGL J2035.3+0354?Ù\ég.¯¸À4÷Äâó¿À:éʄ0'À<Ii¦ŒÇ@âÝ¿
qƒ@(ˆÝ‰³s?Ç˂õ¾2«?™3èòŒ$?Ó5`F²?ýwVô-ŽÙ?ïúÏtFùº¿èΞÃO ¿ç§PÑÑ¿æI´´¨Ù¿ïÿæՌŽï?ïÿ˜ÁØRUNASNone?îóN´C%?³hmv?efc¸ìX?`%7Ùuã?žé]7ÞV?³ú4œ¼O?ïsíÄO`÷?s–'¸…Á?n¿uƒµ5½?uÓ:åX-Ä?‹T±|,È?‰Otaš²p?îñm¢^¨ò?Ùøs2–?{̛˷FÓ?}Á{ïêP?šß$ÃLÔ?‹"d?î²í5" ¼?gƒ-­ö?uœ½cõÒ?[ߓ qª0?¢"ÿ?¶…?!,:e•?íèÁ³Ð7Í?®Ö¤öÎé?u!€9?rÅ5ùg½?®Òà"Ù*#?­ñ¸¤Ø¯2?_¨Ôl?¥†KéJwl?€¡éÉ+³Z?Žâ~"ú[M?£m—1VÜ?¡áD"ûŸÌ?îD(wÝ ?•ÛL'5êK?2øÈÏ¢J?~åW#ғó?§pºT 9?"ÚÈÃ:ÃD?먼åדX? 3ÄçEáñ?ö{§(>?~¼W…29z?¾»I['v?äK½š_$AGN4FGL J2036.2-0207?í>LõY¼À8/KøüրÀ:¿­FÈBÀ<dLÒJ»@}Š?©r@ï !·"?Ðx $Î?Ù{Tà2@Z&–m@Ý­)ï<¹¿ï§Ù}µ7…?ïÿáÍì¿à©ß'1.¿çôïËÕV¿ïÿõž}.)?ïÿxÃÐ¥UNASNone?î»cÿa}&?¡×µæ	?'ÊÁ:›Ö?'ÒX¿ï±?–Ⱦþ¶‡o?•Ÿ™€¯‰?íÙÀàR?®üÈuÌ¡3?ž´9щª?¤v2n>+?£	æbéçâ?œëã^ ×?ꀺ'¥ž$?ªÚvùQR?¯éÑׂñ'?Ÿ÷ð¼ì ?¼BŠ>Ì?¤ÂÄlHV?í5öðÈæŸ?'Ë̉Àdˆ?£Rø[­"?†»Mžnj—?©M˜"Tîì?‰
Ad¬Ûs?ívö1?©:2#ä›?©Zs¡´Üp?¤ÁË(<G?ž‰ø,T¥?–ÂÅÌxJ1?ꜜDž?Á4»ÍºÍ5?µ7ŠZt[@?¹ÇãÖ(Á?º3È‡K?²8@H?è{§'¢ý?±BhS}5?´Jä®)™?¢æ¦1•iØ?Ä
cí݋?¬÷µ®£?èÀÄ–?¨ïèë"?¶8¬#Fò|?¡Öz®C‹?Áà™®ùcj?£JÚÈËÒAGN4FGL J2036.3+5642c?Ó«Æ2åì•@#Lµ»8PÀ:T˜ÜÛ7ÊÀ;ã·½q7@‹«(7V®@JNz·VC?О¿#@ø?ՈE^XûÅ@osۙï*@,ªžP8?ïÿøãú¿ÝòÅÅF››¿è6ÝâžÆ¿é@€Þ·°Ü¿ïGY•?å@\FQóéUNASNone ?m[Î?ĈÔdñœ:?'¶ø»mGå?†Mî:ÿ²?Ùá7šmvr?Ċ3]ƒ†?éž3>=IÚ?ÀCM|à{U?¥ó¨éSý?¢÷@Ý?â?Ä
kÚªÂ?¼hœêˆý?眸÷œõ?®(ø[kÃ?«Uô=Ô÷¿?–!sÁcz2?Ê·Ÿi?«ÞJ0wW€?éîDúŽ"›?œŽ˜¹¾¶?¨µî§Ò'@?"{À74—?ÂpkšOD?—dڔwÜ?Ú}ٌE??Å`Üož?˜^d¯ð·?'H_«'\Â?áþ P!´?Řô+1¿?àéýŒÞ[?Ì豶,2Ÿ?½ÁûbŒg,?»ÎÔÜ2=?Ö»†
 §€?É÷`'D™@?á"rB½"Ë?³öþŽ5Ä?¸ÄL-ó1?¡£üԝ?ÖƦ¸ï~?³
MOc÷i?á\vPÇÌ;?¬€µ8"Ìp?¹•FN02?ŸP]þïÒ?ÖáÁÉìü ?©Þûf^MIXED4FGL J2037.0-2826¿ïܽ&!ãçÀA3»¾‡¬À9âÓì{¾½À<@xã@¬˜@ßÿÆÜH@âE¿ý±q?»«É᤹ø?½ÌR֑?þ˜ªX-¾@%ô†O:¿ÙlÿiK¿äsãýjúJ¿æay,;È-¿ëeØÂ#{…¿ãÈ:@¿ïÿCÂw‰NUNASNone3FGL J2036.8-2830?ïô7Q6:?I )ó;8?'|´JÞåe?…5Ä^<º?SñúG¾È?GáŽÁèž?ïÄ0ωHF?~–IM¡}?Ij7Œç?QªhWX½?zÆ*ã­µÃ?|>, õaú?ï¡å©és?|BÕ¢¿I5?`ÀÊÑ'ö?l8ʒY
=?ƒV…X©Q?xŠmÒ?ï¸ZB§Ö"?]}¯{Û?X6?Š`ø?=X{XDFw?}ÅNÆ
P?ZHûƒXäm?ïàçáG¥}?dÉÌYÏ‡?:€Š3?1\!ýå?kÔ[kÉm@?c»¼cÝòÒ?ï(ôC‰?ŸïVˤêÂ?avè[Ÿì?oôîÛ?˜½­5‡ë)?ž'¬µX¦…?ïDCñòK7?‰$N"—?q	ë!ßÁL?xpªËç½É?"5ûzgÙ?†
(="òx?ï2Dr˜`?~Lãj>~?qwiÇ°Šw?^k—}¡l?•Y—@»ì\?{\'s•AGN4FGL J2038.4+4212?yy=¯?á^wïû¥þÀ7çÇҒ¬À:6ÃákÀ@–¾Xéò@9Ó{<·@?·ÿvä܎?Ø+L'Œ@ ¤zž+Ð@‰ý¡O?èJ*Æ}'s¿Þ/–Æ€'q¿èHüލi‹¿éº\‡ÀSB¿îSfQÒ[¿É½‹¦¼Â¿UNASNone3FGL J2038.4+4212?¾|A•²Àm?ÃÁX°d…?⬊/qf?Ïe"à?ÓÛ<bm?ÉÖès`8¿?¢
!ƒ`ܵ?ª~cF±?⨓¿\n7?Ãñ1¡ôÃ?Øm4P¿‹?îðýÈ\?Á	³4AÈo?®7¹6Æê?Ûpáß®{Ô?¶š"hÍÕÔ?Ü
D†0Ÿõ?¶Œ¶ûŸá?'Îfm®j?fjÙ¹Ùx×?Þš6…½?©F"M¥0?à§zº¨ªP?¨ÒvÚÒÉç?²V—kŠö?Ä%iG[?ãsº²÷l;?Ï=z˜ç0ë?ԗ4ôm>Œ?Ëâ•I[qH?ˆŒÎÆj'?š,RòªÒ³?䞵¸37»?È®FÔ¬Ê?Õþ.3]6?ÈnXSºM?·Š;]Z@l?©)(ÕL¨C?Ýr9<6½?»
h&âÝ?Ü«V￯È?ºŒŒôMLí?W	2 :™k?C6•¥§?âeµ6¶¨ý?²¤™–®G?ÛŒ`~£}?±ú'Ə+MIXED4FGL J2040.1-3137?ësW9'ŠñÀAèAÝ!êÀ:¹Åԋ0À<<š	+!í@ÐõšKpA@š(»
,ª?Í徶3®-?Á·-[?îÄùdŒW@>½õŠ±?ïq¢"¤À¿ç]tàQ¹Ü¿æ 0÷ïF¿éÌòŒyöf¿Þ†õw/¿ïÿ°_ïÉUNASNone?ïÒpµ¬ä?o^»í=Ë?GûÂB¼Ç?>uyž†œj?sÈyöÏ÷B?m˜‹Zô8¾?ï…ÍæÂ7?ˆ=çFi©Ž?f2ʪÎO?pŠ«Òc?ˆÿÓ©B«?ƒ(ÀΜǫ?ï
M÷ÀÒ?‹ètÕËì?y7`óï~8?{­^z~µ?˜hŖk ?†©‡ý_q?ïu¸}NN0?oF	e`­A?aQbÎt¡?I­^íØÕ?Ž=šb È?l°¼PÙø?ï~ß9r#?‰áҝ,?\rfn…Ùó?Tl@³·ò‡?Œñ;fêb?ˆ³ÀÑٝ?î¤ …¨îC?¢jԎ?xÊwQ­2?ˆc©kË_w?¢¤¨·áܓ?žæÔâ?î	£i;?šøÿƒùâ>?†ÛòÊ?'êèJe'?©âÒ§™?—ŽQ.IS+?îj%®(ó?Hâg«ÅG?våÇ9£Ü\?gå³¢K?¦€î9õhN?‹:¸—ônvAGN4FGL J2040.4+0312?ÜlºáYÀ6jǸÕ¦À:¶Ø¦ãÀ<5Cu –
@ FKé¸k@A3æÉÎ?Õjpr[g?ÑëNB-L?þ×]I‡2@St^v­Ü?ài
à"S.?ïšÅ³Ó׃¿ãúz_l¢¿áÎjüÎX¿ïû¼~Ëâí¿ïò&ޑoUNASNone?ï›7(‹:?D"Ú¾Ôœ?}ÆÙð®Ã?r"'ìCÇ?—zâŸGž?‡­ùñ°ø?îåPí‹ç³?š?¸5íÌ?†ùUåçZU?‰ZÒ$Ã??—Ù7T°$ƒ?'xԖßnÕ?íú;¥ù?™'Ϭáü?"[ŸÐú¶?Š/ÈgçŽ?¦ÚšUç?"yHµ3O¤?ëëɽ¬Q
?'…ëë4¼¬?¥ÕøÅyu?‡Š@Ža?µ¶µ°NÝv?‹Òb(>¢?í?b|³'?¥rhÍ$ß©?–ð;"‰G-?Ž9‹¡e>>?°HÝ4;*?¡YÌêÐÝ?í	©ðåìë?±,ۀªñ?Ÿ}‡*±Mx?¥–)¹þ7?¯¦Z¼ž?¦'1½ÕG¡?ëüQ-U_?¥îlßÆ1?¡ø'ˆº@‡?".˜¬¥3-?·#T284Å?¡ð"Íé?è-½·þUþ?¦QnR[&?°Ej¤›?Ÿ}¡Ã"?Ç&{iض»?¢§‰ôÅk-AGN4FGL J2041.1-6138¿žÊzÖî‹ÀBJ»˜Çâ'À:²Ìœ%eÀ<žÙç@/å(
eC@_ÀY÷Ã?Âz¦r	?±¿ÃúÁ'?ñ
£ÇðÄú?÷6¡þ»Ý?ïõ®£¿ÕoX½ÜD¿ã$À™+¶¿äïþ®Ç¿æ¸ž¬þÑ,¿ÐÀ£ÿN)YUNASNone?ï èØÇ?¿8d²ö?Gφ[Úã?>ɉ0¬?†HÑuÁÍ?~åþÎû5?ï/ð»
úÒ?=~`»¡?vji_ÿìÍ?tò§2O?"gNA!J?‰Ü軃?ïE]{(?"Nµ¼I?nÃ‹Œ»è?kV…ü6zn?"ˆãü¯·•?'Ԑ‰§="?î Jð?îW'Vu ?'BÅ=š?nbH"?¦]<"y?zS'o¥?ïK•SõÝ?Œ#[#Ã?^Ñö æ¼?S©'1^Óe?"°
ó_h?‹9û=<eP?혵n{"?§z¯UöÐ?‹øÛÜ?ÕgÙYª?¯·@uýî?£ìMË®ÍZ?îË£¢å{?6<ۆ+±?y‡téŒý#?uhL
Un>? g)eò&?‹J'†–*Ñ?êÅ˳"Žå?™÷֏w?¦f¦m?Š¹ßû¡Î&?¾Ío_y ?˜ÐÆ$¾°'AGN4FGL J2041.1+4736¿Ò¼¬A®Z@¡QÙçgƒÀ8rZ¼8¨À;1hWØ.@˙>ªà"@ÊåN?°hÀ]ӚÇ?Ó*Y— @ /ˆTÍ·®?ûË°å"?ä¡þíÜ<¿Ñh–¾•¿á0³[â~æ¿æ*ü-¨…¿ë'€!£hпîmm¡n$KUNASNone3FGL J2041.1+4736?wþv?…Ò–?xA$ÎƖ
?ê²ÙK‹CÀ?¹z¢¼æ¢L?Ät§ .¸i?¸â=µ(;?š1
Yµ?°v~VÈ
Ë?çKK…?ÆFIr\5W?ϒÁ½hðs?Å	O´ô
?°¦*Ÿ"â?¡]Ÿ>/vÌ?è‹ÙâBÞ?°|ý\°±Ã?Å}†]ҙ?«³n×Ï	h?£J¢ÚmÆÃ?€_gD¸æÄ?âON[ÐØ?£"óNŽ$é?Øøì¤Oø?£µ\¡ICô?s2ƒ(n'?h|XÎÓ2?êéøŠÑæÎ?¶û[«M?þÀƒ¤v?¶¢—lEÑ?‡®ö¼?p˜ãI
?棫ë­À?̌YïNpÀ?Ñû7ÂÃï?ÌÒ\{"ƒ?™ä!Ycý?"JA-ö–?ê‰9ùå£w?°¤Þc{?ž"ëý%?­Ã°Á#?…)¦Ð5xb?f¥Öüm?ãjRô?ªÅó_uÀÓ?؂à
Fe?ªÑ3ӗYPSR4FGL J2042.1-5320?éwm ƒœòÀBãŸÂ¨†œÀ;RÂ}¾qÀÀ<·ä¼­šØ@ 3Æ 
aƒ@T@C¼î2?Ëd¢ÁáaY?"píÓ؄¼?Êg|;ôº?ýW
Éĕ?ï[}¾Ú¿æh/ßkµÜ¿ääo ÷±Ó¿â¢)?êPÁ¿ÅÚ»!ÿ"/¿çNV"uUNASNone?ïü°Ð²?n]Y‡Å?=l©¼4é ?/y'€µ¾6?|K+¨G'Ü?mEàrèž?ï™<~_¾?…ÙfÎ7¨?]dˆy6{Ö?d?¶×s–?†méK"?'ß3øB*ú?ïQ0U¢Ê?7&@\?µ?aGìØwÒ'?`	yYï?"°÷­kː?}‰®Dƒ?ïhžèZi?r&Âì_w?R/ÈÐ×Þû?<ù9§ƒçð?'܏"[aé?r
!×?;Z?ï|Pu/ÏH?ÿh8R9?O±îö?BT–#ÜõŠ?Žòç£ǘ?…@ÑÁP/?ïàg*Óá?™¶AÌÒKÕ?e¬{eÕ[Œ?räg­í\?c¬3
€?—eZ{5PP?î·Ä?`?aÿƒÁ1?eVÓ~ö2Õ?`"ûÛ
Ci?£9âX]
Þ?.iÈÃ?îí¥¬Ä¼?'·'T¶#?h²œCÈϹ?_"e]Íõ?®eûàË,E?'$'ûjšAGN4FGL J2042.7+1519¿ë—Œÿ$À0F[¦ïÃrÀ:ÈLÃ'1À<a¸Š©@q®óñî@꟣žÖ?ÅÒVúb²'?±ÒH·©Ïó?î¿>¿Xp?ý%"GÍÊ¿ìà‡)T ¿Õ¼­šØ]û¿à}Tß«KÉ¿å@x`cíæ¿É߄_u±]¿é\_UÑUNASNone?ï2që~?‹xc[sÒ?S‰¦¦­1\?Dfg5>áG?˜y(;ܚ¸?ŠËnp#"(?ï—âòþå¤?Šxçèõ?_éÁJȱ ?f^:A°ª?†
¶Rù?‡ÍTÁ:?ï1Ã*ð7?…ÐQ(Ì?l¿vkJà?oãç¾9:?–EÑ\!Á?ƒ/ð,&:Y?îŒx2ãú]?€Ù7¾FÎ?fi8Û@;…?QœoL•
8?¥ÑéCtt?€…h€67?îœî¸¯ß?¡ø*We?iÊpS0ç?€[G§?¬™ŠuÕ*?¡'Ûùü¶?îç=¬º?¡y*›+Œm?q`%*A')?'O8 Nc?žÀUFã§?ŸËs=ôÉ?î+ùTâ|Ú?—š¼"Ëw®?xö,˜í}Ä?w̤|*VÃ?ª!¥!z2¨?–jb4ؘÁ?ë'£A«?Îªƒ²ã©?~ÏJâƙ?q¬Á¡@ô?Àʪú{Aü?ˆ·ZZûŠAGN4FGL J2043.3-1520?ìëð/
ÅÍÀ?sBí»ZÀ;"2.PucÀ<wìÔªà@ 2¯Øu@¼Iº^5??×£e_Ö)m?¹ÂH9€?åó s'õ?þLjKù'Ê?ïÃ[Ÿc6¿æ
d(ô¿åt%kÊSv¿Ü W xF¿èEÿ©þl¿ïþ^à`'ˆUNASNone?ïÈÛ¿·n?kØêÜ?A{Ší~ö/?3lՃˎ?yÍ ´üX¤?j'TÍ×ú«?ï‹®™
¶?ƒÊ]=ìe?bEف¨Ä?h©'s?Ê?ˆ­'`D'I?€.5*I…?ïaàKs‹?€-×RY"?ià æ<2?mÑþ'ðö?¥ëŸú?{áSÕZ´?îèö'ݬˆ?wFöÇ?nð7"¥–¸?QKxÔ¼?Ÿ&°Uä1?vHS4ì*?ïˆü(+?ç³3šËl?PÐpóî†Ô?G-w+¦×s?‹¦çéfi?~r'íÈRd?î·Âm3›I?Ÿz¢~2?qúï`ÿ«é?~Š0°¢û½?¢D{Bâí?›4[xâïî?îùÐÒ|q?‡Ó–ðÙÿ?sz†Åà¬?s(LIŒ•j?›çCýxÍ?"ãÖäÉY?í,U.Ář?"W`´×ªÐ?z¤xS"?oò$×o"?´óA…½a?"òEýò%ûAGN4FGL J2043.9+2051¿ã¤zÄIùýÀ*ŽZݜ'éÀ;;øÒåÂÀ<«qøjàI@†å'Á@%Î_ª?єDuû°?ÝÝá<ps°@
e:í;Ø?üãô0¾å¿íÜiøÂ?ïÿ¨Â+‰¿Ú¢Ô`"ë4¿é\'!֝¿ïÿ×ñÃý?ÒDàPãUNASNone?îXHè•ð?¾H
ìÔ:?ÁiɱI?ŠâyòVÁ?¢Ǝ¡[?—ت\§¤3?ì¢ÚýUðf?¹T¾°?Ót?ªEÑ4Å?­MÜúéÖù?«;W
Ú?°ÉXjxv?éŠX&:Y÷?­ÒŸ¾"‡$?´mF-ë8?¢87Ô؉ï?¿?ø¾m8"?¦¿Á`sb?ê­MDp68?™Ëàè]ƒ?´Z@ð†Ï?'êƽ&,3?¶;Tìãºò?'–dÅwO	?ìßù"HÝÈ?«àKA¸UH?£¶/Ûȏ½?ŸIs¸õ¯Ž?®J=ýÞÇ?¥ŽjÕJš?çØŒ›ç?Æ=ä7Þ¤Í?ÁQd×E Æ?ÀõÎے.ä?¾!ñ8ß<?¼mPƒƒ¶6?æ÷öK¡>)?²[ªv"Öv?»9­ͬé?§fD¨RN?ƃPR¹òf?­¿Òª'¡n?äâi?«FgÜÄ+?ÃëÀ$j:?§}"Ù Ë°?Ìe‹óÇ@$?§·Þ±¯B¬AGN4FGL J2043.9-4802?ï)Ÿw:ZUÀC$O"}ŠÀ:a'W«¸€À<Á#і`)@݀$¨€è?ûChjL¤ô?ÃOÜ÷'HB?ã"BwsÔä@ob?ùó:¥|¿ï±Óým©|?ïø®6Ý¿ÅUP~ó{¿äd­³,¿ïÿÆTǏ¿î‹EC/ÑUNASNone3FGL J2043.8-4801?Õb²…Vt?̾‹°;¶S?äŠ×)Б†?Í1BЫC?îï¤wŸó?¡Ãx'¦µ?Ä[ÎÔ?ÄE1ø˃L?çRӒõ̲?Ǧç%ú¡­?¼±Ç@yuj?³üY:¼Ï?ˏqlB¸?±Ì>,æ‡?å–´!ÁW?´ZL­8Ð?¼1	|o×?¥zÚ}ï¬ç?×@Üéû[Ö?®‹Ûi=?áQ""zå`?±	Â_V>à?¸s{E…@'?—·ž[Xû?Å"÷âáGi?¹6¾"6?é~T.Þî@?ÄŽÊ!?£ŽÝˆCÌW?¤éøýc`?²Uæk£Iî?·öµÔ›u?ê.¡ëžx?§FýÚ?¼5
<³©T?µns:G?(?»ŒXúî?¦á§¬*5¡?éUP¥¥w?°¡êÏUä?º?îÔÙV?¥bgÈ
ó?ËêVv'
?¯jª:­?䒻ØC?¶u‰í5"?Áʽ(b±?¦æ"`¥ÆÉPSR4FGL J2045.0+4202?ìÄìù½ñ"¿à£öíóŽÀ9s?VW$ªÀ:ujhS@ Þ8¯õ@ªõ&ˆ*?»ŠgbèÑ¿´y€žP¸?÷쩬6TP@ÂúÅX8?×îyZ^ñ'?Ñy þ'bÅ¿ìv_"$m¿çZ"ö¥
k¿Ø*Hiü¿Þâ^D)UNASNone?¸ÝYhbP=?µEÊ=ëì?'ö‡™Üqp?… ©uˆ,?ì˜z´•ã?¶4OÌË£?ԟ­ç%`?ÍE ïµkB?ˆôx¯#«?"0˜Ë©¼E?åLW—°Á?̪·Õ€
ã?؏Î#—'?´¤&#‹Þ?­¯Ÿh±1?žªN{S#?á撞Ü,D?´_a'vâA?áor˜g¯?³–¯hh}?u}™̚?`â<1öÓu?݅*¶%Û ?³ƒ]6Œ»?´Š¿uY?±ÄNŽ>?"3¥©/T?­å£Tд?ìø[B¾8?³¢=wYÓ±?ÊV-¶>w?ħßbP­?†–D»ÿr?™šJ"YÛí?éqE?Äe«É?Ñ-Â6'a?²àVÑÏ¿?­3Yú–`^?œ£NàI¨?å•éDì\ú?²²/ª4ù?Ñ•lI~?·¦V¼?'b®°]ÿ…?v^}aq3?ç3ª5<£?·!Ü&d¡HMIXED4FGL J2045.6+2455?ìŠg0÷³À&Sü–þµÀ:í§þàEÀ<L2Æü©3@0mUÃÖÚ@¬¤¾Éç?ƽRÜEæ"?úhDµw?ËVâðz§@¢‰,d¿êµ×ÙôÓ?ïÿH 荿臦†è½¿å"‡…¿Öû!sîf¿ïÿ⾦™\UNASNone?îé<w³?ªNzÄ8Ëñ?b6¢¨U±?ZN»kzÉ1?®¾æË?©øüæÑøß?ï'rWz)+?™TE~Cº°?=Ïõ:9¢?M±'ôÛ5?ŽtêgÜ@?˜ôôÆC'?î–{†Lús?'y'Œ‡™Y?o¼Hñb¶?jÙ¯?¤œƒ&¢Ô?'¨Ë®g?ï'=mQo½?e±ùc6Ò?TVS.bõ?>B×´L«ï?‰%Ú7Ìþ~?e@7ä®üé?ìѬc(w?¶èUë·!?wÕøé5C?uÈɐâÐÂ?½ä|IÓ?¶€àÁ‡…?î R¾ÇY#?±ó!A»ƒœ?Q [ášg´?fºÏÈßë?¥mÑ2Å̔?±½Yöø?ìptù•ò_?£‰'XáøÁ?€â
ƒM¶B?wÚÆßÏä?º`€Ÿøƒ?¢Ó3Wì@?îÛ%©÷y?'ëƈ -?h|"s'e?[϶±4oc? ÅÜêÕ?'B¢,‰AGN4FGL J2046.1-1626?ÍE\ɍ/ÜÀ@Mz$‰LDÀ:n"B€À<~3Ѿ¤@<]ˆ¿?ÿÉ>¢Òþ?ÉÐ1[‰"?Ú`?»ËÈ@ÛÂ3×@®Â+ß?é:?A‰¿Ýc5ÄÝë¿Ó>âéĪ¿ålb©Ã]¿î65{âÏn¿ïüTyÔØ4UNASNone?ë_OPõï?´¾íR]­Ì?­+H§:v[?«!ÿÆ?¶oã'm!Ø?§ý«Ê›/¡?îI¤D©Žj?¢½{‹XÎ?'³OÊ®êƒ?"H´¼Å¬?¢Ф?˜&ðVU&l?éònÒ(n?¯ЭXƒ?½a.ÝÒÈS?¨	ꔧÐ?³Z'	ç¼?Ÿ-/pØq?í­ý¤[¢?ås…Y?˜¯÷'âå?sŸùÀ÷?©Mº:Qt?z°HÒ=ºJ?çiôüÒà?¼Í—ÅPy?º!.Vˆ*?´]¸p^?ÅG"ã–+À?³Ï¸ÆwÌ?ëŠké)œ(?¸-æ¢ÚÓ?§ËÉEón?®!°Ã҉?·Æ¼™º?¬â￙r?åù'i?¶'YŽ…¢?É0uÔ™Ð?±÷4³F–?½ÕÜ7pQ?¥+5lV<
?꿜Súý?šHM¥È?¦¦e0»œ"?‹wýQIÕ©?¾¯êÏþ@É?"ŒçïÙeAGN4FGL J2046.9-5409¿Ê¹?Yå­!ÀC3֝0'À;+m,SE!À<²ãô0¾å@ ìôèâÄ?úÏ÷>^‡?Ô'Jœ±Q?ΨZè	?þvÜG©ã@~õ&`è¿ïUtÁrüw?ïώH,¿|¿ãto=¥}¿ÒæV
ΐ¿Öz±!µR¿ïB¡YºUNASNone?ïÉ>ÝáG-?v?>¿»dÃ?F0ÿÜLÊg?AÍ¢U
?xšq ϼj?t Q™ý£ù?ﮔd?^~?€ ¼{Úa?SgÄi'i?[°nÂk ?îÀŠ7g?{ÁãZÞ>?ïU÷¶ãßì?Ndmçó?g?˚7<?hXT
m"?'Y¯®*Œ?€'íËÒ~?îõ§÷Ö:à?yÀc(·Ú?k•hve?T<ejIÁ0?Ø`?5?xÄ-ÀÒH…?ïŒ}xïð?'+Ÿ¸d?Xà\Ï}ø?N€!±8×Ô?‰Ä³ÓË|g?Á»^?ï_À"ë?™½'Å<e?g^–;}Èð?sÒ¼‡¦™/?œÓa;":?—$?í"<?îÎ.ƒk?ŽÅ´LÖb?kÀÐs*.$?i–"Gƒ?¡a
ÄŐo?ÌŒ‡£¨?írÄít&?"í谕úø?w

_T?m"A:\ù?²ùÄ=³Ê?"¤v5t'°AGN4FGL J2047.5+4356¿ã9pÜX}?Ô7.À\ÑèÀ8ÿ,íiZÀ:Tù]N°@"§âÅÂ@½Þ½ç?ÓÁÚ`3F~?èæÙóü¼@þÓr&Ž@²aôçž	?î_u`Õ,î¿Ôjãêv¿íÛX¡ì¿ç"¸+U`¿ïÿõÿ 1#¿ãL?bUNASNone?¢XÃÊ÷]æ?ªˆû˜{? œÄ&1•?¨b‹U'1š?íЧ'h˜?´t§»Ë?ÇãÇ+&A?ÅÿӒí5¬?Ä÷W9øŸ9?¾ëÓçâìŽ?äÉ8jw¢?ÆÕô5=ñÊ?ÓÈåñzÅÞ?²†Õ¸ÆÀ?Ã5àhX‡?«6¯ø'Z?áNíÅ7O?´>öt۞?°Jí….F?'¦¸ÂÒï?Ï(mù>'?°FŠ­1jË?æ,†Ñjì2?±À?tÕ­?™­c]ÄíŠ?¡ÃQ¶Û?£±2÷ÕãB?ª2BîF»?í÷µ]€ ?²ŸEË©F?°'É
±‹¬?·Újc›çÅ?Í»­{ßۄ?ÈN'"2\?总{ù?ɆaÓüä?Íä@úϝ?°úÌ¿À?Äõ‹´öä›?­ ·}ײ‰?ãIŒÔ_"?³Œ_~8í?Š¢pN¾÷?wPÐÒÿÚ?Õ}ü¸B…?¾e>G?äÖy£§[ñ?¾ y:\$øOTHER4FGL J2050.0+4114c?í;ÓNd^¿ûá>ß8àÀ9VN>QtgÀ:÷b§K3@ˆèœa@s¾Ãõ¶?È?m©%Ó¤?ÍHMv«X@Ǡʃ?ý+Vøà&?áó!R¶¿æK>AÚ
¿ã-ðžc,ö¿æIWÍFoP¿êUÒÀá|¿ívYùp™ÆUNASNone(?×þVÿãq÷?ÇfýùH3~? ó™"ܬ?"»…±î¿?âñšçÍY:?Ç;JƒÜÃæ?Øó³0?Ã2¥¶ˆ?¥ÊVB/d?œ÷'c¾m?â¡ÙӊE?ÂײŸá™?×cRe'¢?´zŒmtE?¯ŒQÙQñ?™¡¯Ù9Ç?âU•È ?´I™5¢x?Ò¢§eÆ>¤?¡ˆY
 Qv?ºH€"A:)?'Áž¬&?ãeœ<"¹i?¢Ê§U/a‹?ÃÃHõ<WŸ?¶˜%¿?¦Y:á€Í–?šÀÎDyµ+?驚‹Ï?¸u͂¯fB?Á®ÜÓ;b?·-5Ì£XË?­e1ú?©ºÞ¬«ì™?éÄ"zyk?ºJQ‡Ý§?ÆîۄJ¨?«u,b?­m?±¾Dß-!¡?™å}J1I?è²-9I"?®©ŒB"w??ºÑø_o?•ßkM"+?Áš­"ª?ž‡KŸã ?è?1ìR?¢el¹ëOTHER4FGL J2050.4-3015¿Ã©yÒµ3ÀBÖxl"h
À;þُRïÀ<€‰Ù25Ý@¼N¡MÃ@³˜Ôw¼?Ñ{nOê?Öbºà;>š@¤³ÃçJý?ý²þ½wÅ¿ïÒ·ÈXÉÆ?ïÿLa¢—¿à'ÆN-Š}¿éѼ ¯¸j¿ïþªà"Ô?ïõfI
5
UNASNone?ïj¸–Æ?"š°.'þ?|½wÕY¥?xV*éiŽÛ?—yŠ6xƒ?ÎnQ[+9?îizuß?¥5'Î&ôI?Í
b?˜Ÿ×^;ç? ÿ¨ñj)Ù?™ÀÙÒÙQ!?쥿ˆ§À	?¤l‡2{â«?¡¡…"Ÿ?•Ù4½‹Œ?²A'ûb0? '¹ð`­?í5~ƞNN?'­ýŒ"Ƀ?—¦"'9ªÇ?~°LÒÙ8»?°je	Ý?Žâ
­è?îkÿ™§?Ã[¬E$?DL'†úÓ?Œ1
~'0?¡à,ÿQ)?˜ExºcÚ?ëWœ…B…È?½|Ží[?§"EÌÜË?°Ì3¡	}í?¹³Q³sVÜ?³¹eU´g?ë*aôÅB?ªw¾ÊÍæu?¤Ym½‡;?–ÉÁ¹ûF?¼'–)ÄìÑ?§›¯r?èåÔ{þå4?©@3äÃjw?¦Ý8ØH1ñ?—
	A'ß{?Ʊ_ØqŠv?§á#ÍAGN4FGL J2052.1+5539?ç|€Î¾áÊ@móùa€À:¹‹U38<À;ô×°´h@ös%@vÅ#‹ƒ?Ðt4…Bʀ?³DS§?éŽmìl¥?ü/_"K|?ïìFD‡ïM¿â¡DˆÆ¿¿êŸç[ÄKõ¿ÔÄ5N–f¿ÞÍg'ߐõ¿íäñ@õh¢UNASNone?æ›ï€'ß?ÁøõiùîÄ?q³ËüÀ?eŸHӁ
†?ҁQÏ* ?ÁÞÙ¿¤p7?äåJYëXÔ?ÃÖÂ܀km?'ÏŠYo8ñ?""Íó. ?Õr¥ímŠ?Âö'y–™à?êÕÒ¤#?§+^ƒ'?EˆE¬Ì?ƒG
û×*?ÂÔ\îÃl§?¦A:4"·V?ëÝ@µ‰˜?•ž&h?ƒÜ¬W«¬?g?á}¬?¾šj0í«?"‰<ÚDè9?ßU؋ê%ð?Ä)vögÏ?€ú*ôj"?t´Ùـ/?à+T4=?ÄÚUBôê?ص‹ƒ''_?ÄX¤±Ð?—¸Q—V±-? ,µÚ[Åg?âçw±Îæ?ÃÒ>ô h?ãÙzóÄ»å?³½¨í'?œËØÉ?Ž5Ntô?֋½gBô
?³bdòõŒ?åN¹àЩ•?« 2ÚB?–dJ.+ÊO?"üÀLº,‡?ÓüG›—m?ª!g; MIXED4FGL J2052.2+1635?ã æÀ1dô!-wÀ;
Á$"À<'=¢"@rò»ÉÅ@UÛpÔ~?ÖÊð¿\£?ïAÊsbÎ@Œ¿ôw5Â@†  ´k¿Èž&܍µ
¿å²¢\·¿áŸ¸Í;‡–¿ïÿyB=K?íöÛ>)±T¿ïþùoÃzUNASNone?îR…(Ñãë?´º3ºdæ?›ì˜cÏ?©õ#Lô	?™Â"_п?¤ë#—7SN?îó³Ïø?©ú•†/G?ˆ½‹9¥*V?˜§
¥AÂ?•*Ê1{ç?¢"Ëé8my?çŸÝ3*?²B ½Q"?Â&Ñ¿¿Œâ?«‹©ú¡?Á¾®Í™Œ•?¨™¯ÕJh½?ïJÖr½â¤?†}×àë×n?fß"Ï]¬Ì?hJԒþo¾?"ÉMU7-Ø?"-Hþ@¡'?ìœb¤Ô¥?¸ÝÉ×÷d?©kÇëÑ1?¬£yΫ?¬Ô풀{?®î–"XK–?ìa…gCÂ?Ât_µA?«ÔÐ^I-é?»uuQT /?¬GÒùù?²gµG'?ã¿Iôë¥?´­>·fW?É4ñ6?±‰7¸YY?ÇÎÑ¡j?Ü?­$/Z¿
?ëΠޡ$l?´MïqoX?–žòZš? i«¦"?»ãvG v?°ú±‡ >AGN4FGL J2052.3+4437¿ï'Ø=Ýö?¶öԈ-
¥À9̌5-À:¯
•øÛ@Ì7Ž·"@"rä#*§?ÅÃdCK"8?Ý»ÐZöƛ@µQþÐU@<""†âÞ¿×°Ôßøà¿×¿!='\¹¿ç*7Á¸F®¿íÂÝ_¿ïÿºà¼ô¿í¦.}kæƒUNASNone?·4'qXÉ?¯°¦™ç?͒IZßA?ÀÄW™€*n?å´ÛZóÛH?ÃÄ(aEP?²DákÌI?°õŬïx#?ÂG1Úe:?³C"Pð¹?é%—[Ñ·î?·XûADçè?Îyµ»/¸Í?¯ ¾oõ'å?Äç"Å2_à?©œã"Ô&Í?ã'±_çyÕ?²
jˆ9=ò?±
n ÷?ŒüíËõâ?Çچm6å? ¦fÙ˜?çè	dÇ?£M)Á~ìÃ?©ûíÇzDÃ? +Gçâ?ÊY¹m'(l?¼pOš[`?çÉÒÇìù?¿£"i:…?›Þ»‹Tä?›'<¹Lp?ÁÖ@bŠ}Œ?¹;¸H‹~?ê«zCG†?¹7Ÿ£Í9?ÃV2[òÅ?§x±0}åù?Çù1©40"?°Z&y"Ö?å,&þ,ÒW?´9õp	F^?¾`šÁÚ"?t†):'?Ì÷&+?­z6}§?è>(l'¤?­øn"–…OTHER4FGL J2052.8+5739?ä~¤Põˆ@  ¦°)(À:ÉÈ5ŽWÀ;Á¡ùºk¡@	ý½/ ×@-°ê7?Ä驼ÒXÓ?½½Šåv¼Ë?úB¾ÁqNø@V¦í•?èç$œ—zÛ¿ã¥jÞR¿é·à†=¿Üœ›PÓØ¿ëùoÃzn¿ïÿÚ €UNASNone?æ­sý9?ÁfÄß\`B?'Bëo̬ò?‡‹nÏÈ$?Ò¦va[9¸?ÁGŸJwaO?æñœh½?Ág²¿ý?žËaÆL2¼?—¼HOŒö—?Ð0ª…-?À"L;Ù?é­®¦
*?ªµu'Û ?¦)Iýßp<?–kíӜc'?þòéŠ?¦Ð§­'Ý?ë6äÝÝØ?'쥸¿WL?¤ˆåCö€Ï?€6¤ÛÚÅS?¼fpf3U?$A»§¯‰?âO"¿ê¢?Âp)?¢Š8W¶ç?–J͍úÅ}?ِ´Ì-ž?Â8ª\pªs?Ûº£Ûξ?ÆØo§Fš2?¯ñîÆüç?°Æ›øßôI?à#%Ä­?Æ%ʝ{.'?ãã'mXц?²vD|rš?´ìχ`]Ã?£VÀ¸"Ž?Òý©CZÈ£?°·™µ£Yo?ä'c:?Ÿ†?¤Ò~1q,·?ºÄÿŸ™0?›j?OPi?ÐIù£šyh?£»m4þè½MIXED4FGL J2054.1-4054?äJ_!x ¦ÀCö FÇd®À:A…ô¡'À<_Öq'<Ô@´6"¦É@"*ú?¾!-¢$­‰?©s€Û¡k?낎»F"@n_.8Í?ïW¡!MW¢¿å'"¢‰­=¿çÞDÄU/¿áwáî-¿ïær$àŠ¿ïÚ8?ânUNASNone3FGL J2053.4-4052?ï-˜ßú?¼~™èÞ?}XœC{l?¡ùíQd?"	ã‡?´w'¯c?ïXþ͌ ›?'{j»|ñ­?rãæP¢Ëð?{á ž~?',Ã:‹?ˆV"ìu?ï…#ë†?ŽO"'N•?³Oë•?'´ '#TÈ?•§Ý¼éh?†eA6üÍc?ïpTIê?uqQ+4ÄÕ?‡vwéÃd?iÅÍZ…›?'öÄkJ?l|ª³
ò?îÍy0 6à?°ãô†¥ 5?‹:|[Mâ?ž©ö"ïK?˜³›É*É?¤}G-¯ô?î:ë•Ýí?©þGšÓ"?ƒä1}†•?"±…Ϊ€C?§X:BŠØÐ?¢Q\WÞ}?î'ÇŒ,Yá?"åìû¸À?‡¯d"ý!?"Q|3'*Ù? ÷¦âyÔ¥?e™'Š˜Ò?í¦Çþÿ?'qÚQ´ls?Ÿ<h…bá?‡ª×½=N?¦@ûøÓ?…ŽÛ‹½ŸAGN4FGL J2054.2+6904¿è}æW.Ý[@.'ÄupÅÀ:Lµ›Wß»À<Eþ7¨ã¹@&˜®²@ç~äâmH?ÂF­¹a5$?Øó;Ì@ O‹XŽ?þo'€EŠ¤?è(wŽ'ÿ¿Ä®QM¥¿Ý·A 3fµ¿é'Û¿®×¿é"'?h¿ïÿƒ9UNASNone3FGL J2054.3+6907?àd~óâ ­?ÂoM. Á?Ñ
=Æ	9:?Á%æú–H?ÌSˆ¤e
Ø?¹›?-‰È?ފ»¥ˆY?Éæ	Ÿ;1?Ö¢¶ÁÑ#Ò?Æc3Mµo?Å¥1M™«?½Š×ège?àmî×ñ?´?Î뀯!?ÓÒÉčA?²®÷':!?ÉÈ¢±i¹?­PøK¤Æ?âõ>S€cE?¡P<›vD~?ËmÕ¬«€]?Ÿ÷F`$?Ƚ1RòŽ?—É­f2Â~?Ó#-ƒ¾2x?¿D-ߧŠ?Ôó´Í҆J?Ä"R¶íM²?×é®oG>?ÁïlVaØÚ?ÐÏØ´¦T,?Æ֜2¿ß˜?à…E5ìî?˳m;}ì?ÌK8µâr?ž',¬?֊«@SØ?µûY\èŽI?Ù¯;¬Ô^ç?¹ö4Ķ?ό2}֚?±‡mzµ[u?Ô-…•'ÞK?¤î‹Y',?Õí˜j««¦?®§@"×?ÕäáÿÂv?§¢ZÚKxMIXED4FGL J2055.0-5218?í/MܒúÀCèA¢a¿8À;>$'ýuÀ<‹î:ތ@¸ðá©þ—@ø&"»?Õވ¡y·Ò?Ñwûd9æ?ú«~3Æ@؋`pÙ¿é'Æýó¿½8¹›¿åãEf­¿âÚ
ݹ.4¿ïþÚ0bž[?ÏJùãÜ2ñUNASNone?ï…É™R?©U:OŽ%?f㠖Ày?†‰@ÓÌõ?‰™+yo?¤sžÏŒ»R?ïLJçќ&?vܝ—Ûtu?Je×­çJë?UD‡Ð¸?xïQÍÇ?sK~o¥áó?ïWg#¿f¢?‰"ÏË K?r¢Ê¦I†?vÁB½ƒE}?jwN2kw?†mœ•ÁV?ïË¡n4?W©Å±†'"?Dáü»`?+ÏaþI(*?w®Ô0ôµŽ?V'–èj?ïYPÂÿÞ6?–ʧåìì?dnQZ{L®?f}G÷¸û3?'Hw z¨?"§O×Ý
Ø?ïQâ؟5\?'¸ áZ¥?`Äg9ƒ-?tÍlQe?"«-"	?ù1ª~
 ?ï_¢k¿?Ísl²{€?vÇÉ_\je?yç•Ýð´$?™âSýÇÛ?»ÅÆü±Ê?ïyí둚-?uÇH³ÿ?P—Eå"ˆ?D^ù‹úÑ?qœQ9@"?t)Ìz•AGN4FGL J2056.4+3142?ï«'!=M¥À!£;u!MÀ9<›õšKÀ;»¹&&Û6@웺Iì@]!ê5"?µðR

ú?ÚÊd<Àz¯@ ì'éSQ@gŸÜ~ƅ¿Ô>$ކ³Ž?…¤éó'ù¿ä-–¦ Z¿è±càO5¿ïþ®û*®¿×']<9UNASNone?—…	N½?™— V]?ìfVîp®?¸àú+TÂ?¹£ˆ…Ë¢?´©EýóÝÉ?©÷.–?°ûk‡eú?梽¸:w?Ã$ÌJj2?м'`Gò?Áå=~]?Á`hQlq?¨˜M"Ïa?æÓMß©?Ì?°¹è)m¹K?ÃR`0R"^?¨ñª~x"Ö? ÉÂ3õ.?ž™IÚÂîM?åM#ý5Je?¦Y—â9|?Ȫ¦Höá@? J•lâw?'ÆDˆË4)?'›`ijA?ë=l¦¶&‡?¸ëäÃx5?À±"Ô²ìž?µœ|d¡â‹?•ZNm/à?Ÿ¶ÞÐæO?ç庴5@?ÅøA9°?ÍÀ«GR5=?ÅC?&Ó˼?³Ï¡|1ÁÓ?¢ÆdÆ¿h?éY#õ}›?¯ÖÆä•T?À´±5A«?©FÌð˜ŠÏ?£f@öìæ?†"pIp	É?èR¢ˆÅOÅ?©R ^DXõ?ÉÛÖ-Ùò?§r+PSR4FGL J2056.4-5922¿æBi÷ë_ÀCp¾´ .À:]¹À€Ž0À<yµIc @˜üsÙk—@Ý_á'?Å6ò…n"?ÉOJUŽ§Î@¢¢&0@u@ãJÇ?ïòÏàþ]¿äøŽ¼ÆÅL¿ã"xKtÈ¿áÄ x°ëÆ¿ïÿíöé	¿ælQaòc_UNASNone3FGL J2056.3-5925?ï;·ùM€´?‰xs
¦¢:?zÓ?ó­À?s'Q|lˆ¥?'Ô0ß¿ðP?ƒ«öLèŽ?îþ×Ê4t¯?—ße΁Ì?€Ž¯ßÄ߸?ƒ¤/h^?—Ý®ÇS;;?îÛÖ^€?îï›Âv‡?¾óQc"y?‡†ÃòìBÊ?†_æyÙü.?–I%Ác?É?…€¦àR[Z?îÄ»n´Y?vƒU'UH?Š$,&¯?gçÑôˍ?šV… O{Ÿ?pº]¢ˆ+¹?î]ýP?¡<ÅãaE?""(ú¿m?&gXžõ?¤þVb=?™ñw7C?í^¦‡qW?®,æ#F<a?'K¸53Á?›žb9¿£?°|,½¡]?¦U1b]<?íQŒ³ùA?¡šö;á ¥?žÞáÂë1?"w·»{hB?«wίÛ7d?˜…Ré±?캴¾—?'øÆ){õ? Nâ!ƒït?"ñ8X?²NßàE"?ŒÂºµô|AGN4FGL J2058.0+3338¿ÒaÖÙ.ô¤ÀU´$_ZÙÀ;-¶Œ§—À<¥"²È@ƒŠ'3õ@-@«?ÏíŒàΌk?یÒÁƒmˆ@	.<b'?ÿüW¯>q€¿ïÿà iA?ï¡ 8Bg?îN™á=@¿âåÃ=×Ñä¿ê³"¢Ú¿ïæ^£úE¬UNASNone?çá¬×GT?¿ËŒÜÇÂ?¶_åƒR…?³çè-¼¬?ÅIYáÙàm?µÔ ãO?â«à—ô—±?ÉUü©çÎ?¥ÁÁƒ|þ'?©Ã¡³wï?×ðŸù§n?ÇH߄ÑÉ?ê#Àið',?¨Ë(̖µÓ?¬´š»}{?š¤}Ãè13?ÀjÑ1WÞ0?¤#ö1"¡e?êžS'¤1ù?¤XÓ¡jWé?²ÇBh«>?¡+Ȧd'®?¸F!¡Hy?˜5—2ì?á܃ŸÃe?Â{u[µ?Âqxééª?¸©÷pE€?Ó<Ké@)?¾x‹†JKB?تnuuð??̼ȆÆ?±9Í×{áÕ?·^‰ôY/|?჏
cJ?ÌÇËuùp?æ4x(kë?°y©TÆ­ƒ?¶Ú+o,y)?£y°]«?ËÁ	¦ƒ=?¬£ëE?åi
sT0?·WULC¦?À'Ú»Lò¢?µÔºôó?ÉØûu<ÿ ?°µ¸ç-D^MIXED4FGL J2058.5-1833¿èRT—ö›ÀB¨ÁTɆÀ;÷sI£¸À<Ý1=­ˆ@%% _Š?ôÝWšÉ?ÑÇ"¾Æϳ?°U2a|Ú?ÑwÂd$ö@j&Õ+ëì¿ïÿõMõVY?ïÿ2æY¶¿ïþÛ½«q³?ï÷݇/3Ê¿Ýí¤2϶?¥'mœÕRUNASNone?î[Š;³?±uýþ¶
u?>"Š²2|S?G²÷m'¡?ª
3=LÅ3?±f¿ßfÑ?#Êh!?ª´©RdË?I®ÐaӖØ?^àò~¤)!?~ê"˜}?§BØnä?èòŽÒ/&"?´^¶¼«Ò?ZT?m3ÚéFd?̤µ×gÛ?´eâ
‹D"?ï:Uùi?‹4Ôʧk…?P"ÙÔJ‰?K'—«ÉcV?—³1<°Ví?ŠäVèUO¤?ïW2‰ó'æ?›åÃŐc'?Lañi^?QLÔ~ÐË?"6¦y3Å?›hâ &Y9?ï4ª‡	…?¨ãQ¢q?Zó®Ó—?€^p÷*˜¬?—ÉÐ.†D5?§í­‰câ?ìR6H'iI?©69Å@ú?]Í!¹ì¨é?m"
±…XÐ?¼÷3z"R?©)ªº'Þ?í=
¯RàÅ?«"¡‡"?rp†c{ŒS?zU@³«;ù?´ð¢"qÖ?«$ÚàAGN4FGL J2100.0+1445?ì=-;¼2À3üæâ!ȨÀ:ŒÙ™cé´À<@HÊt,ù@ç®Tçî@…¢Ëqƒ?҄‡ƒí_ê?ß5ÿ–Mµ@È§¤X?÷̧¨.]¿ ÊŠÛÄ?¿àåê«%)¿æ÷çÝõ>0¿í'E.Þ:¿àèú}	@?Ì$ZR[ígUNASNone?aØt?"'šRÐR*?Z k紘?W}0]ö?…>ÚUZ|?ƒtÐåÙn?îÐׄœî?¯¿§¦EÑ%?œÔâ‹t?¤<JZô5?¡Aì!nY?£DÈDÈt?ì|€|±?£•â«¶p£?Ÿé¸ô[d³?"©Hš£…?´$Å¿vÔÇ?ŸóÞâew?êL‡`Ë?¢aŽì:§ü?²Ì2ω?—ÝÅ@Ý?ºÏ©éüf ?šÏu¼á?ÎgÀ?¡
*ìÚã?{ŸH"H?wÜ¿°òã?¢âhԄñ?Ÿp7 Bl?èfâ:zØÂ?È"9…ª?Á&]£?ÃUö敏Ž?º|È
~«?¶ø²M?êyÆÐ?©Œq½Ýp´?©›«
½ð§?šºæ2ˆð'?¿cúT´&'?¤£ÊÈV>¨?̯߮y2z?³­͆Â8?ɵAÉV©8?µ6Ua[e?Óv'kÛxë?´AÝÍ	AGN4FGL J2100.0-4356?֗­˜v{TÀDŽDR?gõÀ:{®•ª ÐÀ<s"vD)û@¢©"P¯@Ì"û­Šè?Âă½B(?±äÖ?íÛ{@¾>?öÈ¡›@
¿å²À?à¿åN.â´G¿åCì>Bu¿â.'Z·Ü{¿ëŽ'Èê¿ý¿ïÿV"tnUNASNone?î®8.'?­
Õ´'­?g¨Jn†˜ý?y¬V³á†?£¡øs$×ÿ?ª6ùTSå?ï=Ý£´¥?•üØ#Kp?tÅGqªy}?"ö¥²Xa©?"ù¥õ|×?Hø\ì–Ì?îÿ˜çî?'žœOæÏ?x‡›Ô€?z£cî¤$m?™þšŽÜÞ/?Ž®ÒQ4?ëWQv?€ÉÄû?ŠØ§ˆˆÒ?ml»‰hR? ±§Š "p?z×T 9?í1T|6ºÛ?ª—&Ÿ<uñ?ws	G‰yä?kð3ÛÙíã?´þ+ˆê«Í?©îcAæ Ó?íÈk0G?¬ÁlU½0?‡ "éTŠ?».P¸?­''Ð?©g¶l"üò?î'zœåd¯?"ÞD¬Gë(?˺Á?~Bò…¦m?¢—cB÷IÄ?'‹GE.Ÿ?ìhlÉ_?šë¶ËBX÷? þ$>ÀÞ?ˆ \…«¿Ñ?´²£R&ª?•ÂEäêAGN4FGL J2101.8+5044c¿í–îïaw@½šzj)jÀ9ˆÁe}'À:Ø´«m×t@˜^IŒ¦@"¼¡Ÿ?Ñjþ;.Õ+?ҁõuü@5" ¼8@€ˆ'tð?ï¿ø="ßE¿ÕÔ~œéf¿ç|΀2À¿ë8–IƒÑ¿ïúmN·óø¿î2í"ñÚUNASNone(?ÞÃ"Êvÿ?Äç':'\ç?£o ¢¡zð?¯XÞKKï?ÞÏ
gOM#?Å2ß0&¹R?Ý:ìa£Å?ļ:ÔùRM?µÄ³'ô?­i*9Z+Õ?ÝT½O3ø^?Ã~¯rô¿/?Ú¡{å‹&?³/½sB¶Â?Äßâ9½?¯À	3Ê º?ÛT")˳ü?³è³ :y?Î}¬9À?¡ý›^±4m?µºQÉA?P™¡0?åÀqdœ6Ø?£²¼iH?Õ;"j±?À=ØõòWm?¤'L3Û?ŸnR\ÝëG?äM°{Í?Áؖ?Ù?ÈÀ<nxâ?Á1Ì~¦×£?Ãäٍ>[I?À÷4+£b?äÖº0§?ÅÖ;ëÖÜ?ÐaXVü?¬•½¦îí?Å­É ÍÉ?°ð3Ýÿ¯`?⋇Q¡?µ-»Û%´?´$Ÿ2?"@hŒ?¸"ýwÐÌ*?ž)x©œâr?êxßì¨ùù?¡…a±ÔWOTHER4FGL J2104.0+4623?îpžÑ;òJ¿Ôj"m¸j?À:<»+º˜îÀ;¸–ªÑÐB@Îäõãq@:µå)»?ÏUöV³ëÕ?âVr¬MÑ@ó-¤}ù*?ûrA>¿åÜÁ6–•¿âiOBÇ%¿ÞKZÓ¿ènq'yAŠ¿ïÿÿ" 5•?ïðÔ^;Ÿ"UNASNone?ÕRná£ã8?č.o\·Å?·Î¨³¼?µ}õ_Tý?â]yÒåý?Ǝ=Tþ?Ù}#ËÎÜ?ʙéhÂiÐ?«'¢	—½Ó?¨¨TºšÚ²?áˆTQ)Ø?É=zƒm¢	?ÚÓDˆù–ã?²bûdB?ÃÞ+¯[LØ?§ã³Ûb?Û=¥ k£p?±åL¡HƒŠ?áÆ[&ŸÚ"?±bÊip?¶øÖ-›/ ?™L0ªQ?Öµ'?°J~¥u»†?Êegh?ÀœY´É˜?ÆÄæŒÄý~?¾ËÙí?ãÎtÿ†?Ææè+zú?Áôä¥ÓÜ?ÃMš°£~þ?²'0Ü,@o?µ3'/–;X?é0 »e¶?ijZ7%}Š?и['x?¯mS5ù?É=Uê?±ÎŸZAͧ?á·áéãi?´exܤ?Ðv[û>û?±Í8 –?Á!ýb¹*%?ªOZ-¹oÏ?ã|SÊ¥š?µõ™áõMIXED4FGL J2104.4+2116?é%íÙüyýÀ0ъeI/õÀ:cÖ1riÀ<3­¬v0@ &J4'æ@çÝÿú÷ƒ?¹¸‡E"©¿ Ëq>AëC?èÑÌ`–BÍ?û‡«¸°¿ïç:ÁòÔ?ïþ|ý׆º¿èktøÐ`Ö¿Þ±ù⯍!¿ß­j0öB¿Ø0~ã"õUNASNone3FGL J2104.7+2113?ïìÕ-û?n,E|º§c?L}GoË£#??[ÚÁÚ/?z™ìˆÓpy?l"¾M	s?JiºG©?€Á'?'›?S=0mÇ?[€':
2:?|ۅ0UÒ?}5m¾S3?ïB$W¹²?"RªÚM*¹?k®¡£´;»?jó-™t:y?"E í!¶F?'ÀÁ
?îtÖî'ª-?~ðâZš©?ƒ}1J'?g?åàÒc?£ÓNSò†Ë?|Úr
vÓ¡?ïfíÀ•åc?‡xžñI
M?fátÈS"E?]F<‰ 
D?FVø'?…uðíÊe˜?ï/…4"¶?—¹…Ë›?mDh¶kâ?{rñµGž?–fÌpdÁ?"o^õ<æ?î'~K¤2?'ÆQº[%Ù?v™òÏ$Ê?qbЈ,ڋ?¤(îÍ9?…ô%u=@?ì—Ò¦?™_%žWì?™"ï.Ú/¢?†yüˆ(?¹*·wp¼æ?—ĪsÄAGN4FGL J2105.9+7508¿ïþ>i'™@2S^"ñÀ:+Õ£5#ÎÀ<8(¾e*ý@5¥›ÛhF@"}ÔA5?½#qõáõ?¨_¹<æÔû?î˜p9Mÿg@y®$û¿âßßÏp¿Þ)«|ñ¿æ~"4­†¶¿ÞàÙ>Ú[¿áíks¡R¿ëZsž³3ôUNASNone?îÿ€v2k?˜uÊU¥Ù+?mÎ~IÎ?b­	7µ?œV-¢ê??—f"¬yÜj?ïit
=ñ}?Œˆ2iØ?mð¡`µéÜ?p¢¸8Ú~Ê?Ž&Õ!0?ˆ'.ëfE?î~À¿š¬Œ?™ÛìéâÕ?r9Jà24"?röiaôä?¥ÌÊ­ À?™!ƒû{¬?íý]re¼â?ƒ;)xæB?‡¢ãf¹"Ù?eµµÄö|7?ªAoü†0®?'Y•åIz?í¿Œê«ý?¨ùø½Gr?€@èݶO?s¨>®Z?¯ÃÍ-q‡•?¨.Áaô6ª?î_œ#Géà?¢¥¢°Qh"?ƒE)~.?Š€ÿ=3?¥4ój¯ò?ŸOìC2û?íoɇÚ½?¡}—Çýó?.Q©Ì?xËE¦6çÇ?²ŽÑû›þ_? þ6äÀž?êZƒ¡î?ŸÅþx ? Ë(½ wé?…FR
­¬e?Âb†¡ÍÎ?žÓRt'cAGN4FGL J2107.5-1507¿ê'#Ë®ŒÀBn;ÑgfÀ:ø0ÁhëÀ<2¨J6"÷@ ø(›)½@՘ZÕ8¬?ÂaÓY®Çÿ¿»¹f®_Ï?ýî}÷|¤?û}/և`²?Ò¬æ}wúã¿ë¡É¿îZU¶ë¹ø?ÛlKU‡¿æOËàÏ»¿ÃàS<h5UNASNone?îÈÇ
èm_?«ÐúŒ5Ó?X(ˆ€[ËÔ?aÂjAÁD?¢²JÝ¢F·?«7‡ïŒ»?ïtš<	y.?•x{œY?oC½Eá?ýr??‹­	{
?ˆ¤ÏîðW#?íOlé|?£ìúaH?wš®‹{ñ(?z¼Î©ÿ?¶ƒÙ°3Y·?£Ø¡n¦™?ïä*¦5£?Š9•t‡@›?bž'¹=ìO?Y¡hoQé?™¯¨Pu÷?‰"¯Ú'h?ìĕ*k…×?¼nqÀÀ,´?q‡»q—ß;?qç~¦dˆ_?¸ÂÚõHZÑ?»í>mŠ-Q?îyäÃ
±D?¬X/¹M‹q?€šÅóҐª?˜«k†¿U?¤;QÂT?¥	ù@,Dz?ëÈÕN{Ž?©qfãx…¯?†ÄMQ‹p´?† ñ)"ñ?¾àËåÏ°µ?¨(³<(?죚cîçÕ?­–׍ê?&ñðîv2?uMí›9Ý?·>N£Fٓ?¬¿iÕ	FAGN4FGL J2107.7+3529¿½Ø£ðŠ—À A_ˆü"dÀ:~¶H&	À<
ÿÖ"î@P@".þñ@È"ä0–¡?ÈzyBáüà?¶ÖÖ»ãñ?ó"Gö8Öá@  BU:?êDã߸⵿ٍDv§|¿çM}ŒGÌ¿ì	áàÛ!¤¿âƒŽ_©³Ã¿ï«a]*UNASNone3FGL J2110.3+3540?ï¬5)Fd,?wâÞÈ`Ó?D:D–}E~?;D…J8d?ƒ¯[B¦?wë®<#?í㹀ó8?¶ÇNC~Ê?X'fÕF£?iÖIÏâö?·>Ø/"ú£?¶^Ïî:;Ø?î«è¼ ƒ?'/4KA'?qötêL_`?p*XrJ³Í?£¥šÛma?JPð®4y?ï¦=]?_ê`®?J Â)Mè†?/£}úÕêE?"Ï0Yƒà?^¾Ê8os…?ï*ZPGYö?Q,™z?SÐ"$<ª;?KáUÝ1?™w³Øă¦?Ä©–%–Ÿ?éP n€l?ÄW³×C¯?fîï"KÕ?{n5Å68ø?ÊaÅØ;ë¾?ÿ½?ìûËè? á¯29/?'†¤ïØ?zDOÓæf?µÐÓ	ÛS¬? iâ*û?îìCd®«?€[Mç"q?b?Œé?O§?Ûi–<? *¢âŸ?³îߐ+®AGN4FGL J2108.0+5155¿Ýúø!h@N>ò"{À8í̙¡&VÀ:vF›ÅÃÄ@©PÑ~¸B@:ÙºñØö?À\‡ÀSAÆ?ÐßüÉï£@NÅ£ßâ@
¢›Jõ¿ïⶮ}Vm?t¼j¿âþÚÁW"Ò¿ècê?ú@ù¿ëòpK™¿ïõA?æIöUNASNone3FGL J2108.1+5202?±¼¬;+?°ðW‡Ï_?×OŐ?Ôî®Ï5ݲ?â=ÖÍ]c?Ô5àY?ÊWäîVµ?À9…‡¾Ð¶?Ïæd/vÝy?ÉY$ß]s?áPúæ²ô?Ã|óQ.N?̟žX±P?¯†q¤¬?È>¸ý®?¬L?C˜ÎF?âÈjcºÔA?±ÅHúéÂ[?¿ubè5<?œÔœ÷]tC?»â‹ó58¾?–Žü'9?è•
<RA?£ïYÈ%üœ?¦8ñ§Î?¡Œ×I•"¾?Ó¤ŠŸ'çZ?ÎB6LS{ä?äÊ:X7ñÖ?εŒ–s@â?´æ;ŽWŽ`?±ï9¬Þ•®?ÕXOªë¯?ÈlaÊl˜?âٌfˆÓ¬?ÇyçfoåZ?¾jƒ¨&áQ?¤%âtŒ–?Ë5Œ`Ã[¬?¯ŽtAµ?åeLrÊLë?±é*À6Ö?¥Þóá{¿ñ?t¶"Øíö?Â/øØ»ºÎ?¨¥þÚJ•¤?êŒ'HÍ?«èd.³¾OTHER4FGL J2109.5+5238c?ÉæÁÚDHs@	ݜþ¨çëÀ9W"¥>ŠÀ:ÄXÉűP@]±°ç"ø@Ò¹ƒCì¿?ÆCß=g¿'?µžÃúì?ñݸ'#Zx@DgE‹%?îè¹AՍf¿å%nN'4¿å÷ìÀÞ(¿ç¸Û^
!l¿ìӄABÀo¿Ýޘ|84ÐUNASNone8?×y/;áA?Ä
f™Î.?˜=
wmçè?'UqÇN¥Ù?ãö¬¡?ƈ˜ù®?ãD£eÒw?ÂڅҽQ°?¡‹GKe{?žÆ/äDÑ?×EUìèîc?Á•hù¤Ø?Þ †]Q¿»?µý5—³Ýµ?®í†±®?¯zÉ{[?ÞÈÌ%÷¥?µž´§æ.5?ÜwXOÍH?§P‡^±û¶?ŸDËz?yÛªØ}§m?àÊû:Ã?¦à˜2p¨z?ÇV'!W?»r'dÈ×u?šVø •UJ?"ÅÛM
x>?éWÁ0ü ?½¨"ܑø?Ô'Žä?Ãz™AÊ?¬^ži3¶–?¯î'ÊÑ_?ä-Ø3w?ÃÅ0άù?ÐèzÁ?±^iÆÉ&?°Uz1©®*?š:ÝÓX¢Æ?åA|³@?²>ü¦Ï?Çe$°A.|?¢ñ ™Lž'?¨1í‹Ýd?•kÓù?裦dûy«?£mÂõ<ëMIXED4FGL J2109.6+3954¿ÒYÀgÛþ»À¹_í¦a(À:lf»ö»´À<PÍwí@"`´á¼©?ö)`F'µ?ț	›µ'À?ÔÜo×ÿ0@f}þ2 f@hH0p`:¿ïÿ&DÉ^?ï÷
ø{§¿îÃ`!¨Ç4?éìu:'Ä¿×C­¿@r6¿ÛªŒ[¨¾UNASNone?áh»òù¡?Ìs®rž?"18¼Éò??<›ì?܎HÁÿƒ?ÌW*ص}?êÆàÅä6‡?Ãf"dÀN?g°h'Yœ8?{í<M÷üD?ą»D¨ë5?Ãxo$
?è拇vñ?®‡ö"U:?›*!F¾?"qæz²s'?ÈöŒÝ|%?­
ïÀôt?í]³wÄ»9?žQ¢zŒå¶?~å«£Vç?t"P¢Ue?³0•æZK?g8vӖÌ?֚Cp ¯–?ÉWÕÛpÔ?'Z<˜~êÖ?'~ôaB8?ä cKåî?ɔ¬.
™%?ã_vhù#ÿ?ÍËu§Õz#?~Á'­æÿ?—õ	
0z?ØÆÐ)ß³•?Íd˜gâ´¸?ä	®ó{•Ö?³?§Cë-?§¯"äE?š1*þT?Ôö±{ý@L?²z˘Y•?éOïNî,?¶H·5k.¾?›~$Èm_?žI1$Ͻú?ÇP'aÍ-#?µD1±¤MIXED4FGL J2110.7+5129¿ß+,Ñ;¾¿@ƒڐڮÀ98CEÏíéÀ:aÉí{ì@À•ý­ÀB@¬ dŽõÒ?ÐÏòñúƒ¿?ÚiÐ1Ü@
ïB-¡ú?ÿdÃo?ïÔ.öw¿à†h>ح׿èö=áâß¿í֎ín-¿ï÷/væk?ï²Û‰þñãUNASNone?ÖŒnìO?Ð厴'(R?ª3-¨$Žå?¯7¿>9?ãRI_*Ä
?ҏV{ò?Ö¹ñ0Œî?Í^Êï/¬?¿'jjê¬?ºÉ¸ñ"Âx?á
Uº$\3?˳ќGýM?ԗ"K¦òs?³—hèú"?Á#2'¬óò?ªZQuõ?áki5IÊ?µ.j\cY÷?²LÄ#s?–,:6*á
?·böAh¿­?––·À_ÑÙ?êÊ?…si?¡­ÔD?Њº
IÒS?Î9œ¦5֞?¶+·Uü"?¸)fÎø?äø}ƒþ´?ÒÌÖâIÎ?ÀGz+Ú?ÁÑiö?É܃à0(?ÆÙ×aÑ+V?åhzöžàß?Éf™´hõ.?șÏVaX?­=Uh?Ä?ÂÐß(øzX?¯Tixdv¿?å%T`)‹j?µ€æO)ÞÌ?Œ5¼qØ+ó?wï¢_ôÛ×?ºÏf	Zƒ?¢¯otÑ?ì5F!2»Ð?£qÉl¬6æOTHER4FGL J2112.5-3043¿æ3U}"‡9ÀE8Ɔ"ÄÀ8¹}'âïÀ;ûK¯Ri@æDÖ ³?ù?<;±'?«é³@pž?݁b ß9@1== ò¾Ï@'wVM¿|¿Ý¸çì
?¿ç¨eÜÔ¿ÄTÌ '¿àã|aO{=¿í/à˜[¬¿ïÿý±q&´UNASNone3FGL J2112.5-3044?‡mX²ß?°šH2w5?ïãs­h?©;Ñ
 Í(?"Zî-ݘ?¤K…X|À[?¡mòu¦i?¤ûâ¬5'?ìv®é?§¾?´Etx?³"z*[?°ú—ÓtE?Ÿ\Ôëtð§?—¡Štzµ°?êbò³¼/œ?²¡ÌñE¡?ˆš'VÈþ?±èëàea?}\ýÂpö?pÓÞñˆà?ì
9WG?¤~€'õ[B?½¡Æ[;‰?£¥ê	ôuˆ?…¯>cÁZ#?%Úpæ®?ï–½¾‰`?¦¼9ÂôzÉ?"‰nï? !×ǧŸ?˜ôÇCŸ2?ž+¶05ú?ìvCíPâ?»‹#Æ>ú?¶F#að:.?¸ðԇäâÚ?™üƒAëC?"{ä«Oth?êÒ²†òÅQ?µ…'h‡N?Áu¥|.'R?´Ñ—"7ÿî?dg9`ýé?]dé³hDÞ?êøˆg?¯@Ü]?ÃÎÉéñ?®ø¦G‰PSR4FGL J2114.3+5023¿éUÊ5ۍ?òaKßÒcÀ9n‡–aÖµÀ:é×5Ü@£Dîq6@±3™Š€!?ÆÖáM¸E?ЫÈÛ¦"d@×"ƒ¸†Å@¥¤ªCàÕ?ïvŸ~µè…¿Ý[òú³åË¿Þˏ(ýO¿ãÏ¿®2¿í¾‹Ái¿ïÿ ß‰
UNASNone?°S
¹`l#?«‡t½'ý?«\Df¸?¢ã¹V`?ìE8äx0?²C'§2á?Ôr¬#£·ï?ÊEaø²H?©q7E~žÈ?¡ª"Uàõ?ä/–zD-›?ÉÒ«PÏÀ?ØÄ8ÅŒ¹?²dTCrGP?¼ð¡=Qð
?¤¬é»A ?ßÿžë+÷D?²nãz±Õ?ÐÝæ3¿äÌ?ªÚ®ÿàµ?¨ÁË·¯÷W?…_¹®Ið]?æð*Üä?­>õÎÇú?vÅÔìô
?'NÝ_vp?«Á‹÷«®Ö?¢q¾Š?íX1ùZR?¦ãy—³ŸÜ?¿õ'd˜?¾Xªjf ?¨µC"
€»?¨¼T0c2?êuù¢©ôÂ?ÀŸÍ3é«D?ÇãؤhÌê?«âË"éê?À_m°©øÚ?¥ÇO)Eå?åï.kD¾î?°œ"úF?»0gsN"Å?¢eÔƒð?­	"_¶ú?•Tüê?êÈry]þ¨?©IE.¸n)OTHER4FGL J2114.9-3326?֖oP£d&ÀE¬§?tŠÀ:Xš`hödÀ<QuÍâv'@¶²}k:·@¦¦Bˆ?½~ßrۄ¿â±†J‡?ÆÜô7Iî6@»Ÿ/Z·?êJ7&úƿ֔øà|-¿æZ*M±c»¿Í"‰ê}7¿åà• ãû=¿áÆëvÛÿpUNASNone?ïÓ)dʧP?`÷A$ûÉ?F#Ͷï?2"ìV'LB?s¦ìüâ¦?_Q'#@'e?ïÎÌ÷ótµ?r´™_?C!FŸ€?K
Þ-V?v7ŸÝ`,ã?p¨"W?ï"V끀?rDP&´ûÅ?_{žDr?Wgæî´òœ?ŠúяK¯M?p~»™·Q?ïhµZÝÇ?iE1ðª?dÕuÐU/??DôF}¦ãÁ?N°ž580?hõ
í?ï"Px?zPé&Ÿ¦ú?\j÷ªÌ?M´Z	Œ?‡^¹xž?x½dq?ïvрeÀú?Š.nKŽÔ?Q™{ëù'Ì?\G¶xþ"?8-Õœ?ˆ­ë‰q"?ïûŸ78?†{î¤=*'?mAîÄ磯?fSu›!D?œN@Úڏ?"-ÑÉ$U?îkŸêÛDy?"·žÛ)‰?}SM™3ÂÎ?e$׿0åK?¥›—Ÿ¿.œ?ƒ%'NAGN4FGL J2116.2+3701?éüŒ<'½MÀ ®˜ÜÛ7ÊÀ:"܅§tNÀ<=èõ!­@&*yPMö@ê#×u?ÅÒîNý"?ìZ0Fï©@"­`ûH?ùk5X'¿áF´"×j¶¿Òr‡[ÿZ>¿â7WOr.¿ì73"l;'¿ïígwžZ¿ïÿïXzUNASNone?¤—QÀ¼ô?¥<>@Iʎ?äN¯=DÙú?ʐ¢¸ì?ÔÏ·M^­Š?È¡€©ï¹G? oµ½¹õ?©FÉxe‰ ?æZã«-J?ª5 BL£?Ñ<Aò
@m?ÁÒ{¯Æ#2?Êó f°kÌ?¯")§z?âÏô8eeú?³âj¾›ÎÖ?ÉÍ·¹üL?«¥O¹¶?¥j‡¸é¥?‡¤Å¦'ˆ?ëÛL}˜Bh? «X0.â?¶pXÏko?œœªx'?Ì'è$·²?Ÿ°±È–?ãÜ Ä4'œ?ÈT–‡b׳?×I]8Œ°Ê?ÇðšSË%¥?¦¡ìƒ´F?Ÿ7D83æ?çxsW¡¸³?Ç`´hÛiP?Я1†_Ö?Æ¡'–$£?¼»$÷¹¾?§	ˆÂkPÚ?åôürƊØ?´l]Ðòt?ÉÎ{¹õ?¯¦é•-ÄÌ?~.•\M©Æ?jj.©Ö'?íd"½!ç?¡îv÷ cw?²ü¿Ìî?¡+'ňîxPSR4FGL J2117.0+1344?Í€±|uƒÀ7Þs×ÛõÀ:{Ì'‹_DÀ<Dô·ÍaG@²‹'Ä
6@=¢ø½ì_?Æ´©Ýßo?ÖÙ`®ìg@ìJ[mäà@ÃHïÝóç?íœK9¿áx¾'²!¿â<۝Ëœ¿ã¢–b­tB¿ì±–`)5ƒ¿ïÿÿ«FjUNASNone3FGL J2116.9+1343?éøäi.?²Ì"xÄ8´?°a)š}ü!?£mvõ	?¿×¶['mê?ªÔ ¦?îÛëÊؚ¥?—E¯¨ëÓ?‡O5ê•&?"ý‡…+4?˜Úë±YøÇ?'™&‡ÿ?êÈ3*NÞ
?¬»ò·|Šh?³%
 v_[?¡NjØLC?¶™\°X?¢n¡õèâÉ?í
RB̔?†Kjaª?—n¢PöˆJ?q^|ð
?±ÑÆsѺÇ?'Øàñ
Þo?åU£v£[ ?¼È´_ÿ«-?¼›$Àöø?¯ì !¤
¾?Ì[ßÂÑSù?¶}ý®Åds?ì±òÔ¦él?²ðº µ¨?¡ã`°@n?§&¯ÇLh
?±~¹"Sh?¨=Xz:dÈ?æÑ®Z¾3ú?³DÙ¿µžC?Á	ù]Ïi	?ª¾LcRW2?ïM77Ç?©Ÿ,ÓwÖ?éyp?"Q? eü"?¨7zü±¨?‰ZIN\í1?Ũ;ÕD¸?œá}¿æÓAGN4FGL J2117.1-5307?ͺфŽçÜÀE~\|ؙÀ:ˆL€À<'|»@ð–ºìû@	­þ«l*?Á¡ËiM÷?´®!7?õ­·þßn@o¥'(^?߬:›‡Z}¿Ñ¢[Õ¾¹¿æSþÕÞn¿ÑÆU#óпä¢n>÷âz¿ïÿ²gƸ·UNASNone?ïò€%)ZA?H¼Îóºt}?2öGÆ9—=?#<ž¿0Î?VB$ žkž?EКÉa"?ïÝôt¨ì?nïxö§¸?9—í{%œ?DQÞ:h	,?o±(rf?kšå;´>?ï¾Î1{Î?c9ÊÛì´y?QˆšÉ'2?:Xf0GQ	?|6À® Ú³?aߖ4֒œ?ï¶8'²c"?Y>Cà:?X?tàSÉ ?7Š£'¿†?~Óً–Š?XQȜÖØÇ?ïã©oqõ2?\ÇnX– Á?DvëM%?5²]ù9Cd?g8ÕÓip?YŸßæo?ï•q3ýf%?†o£:§þ?J` ü1 ?VË+$?ˆý°ó¼öw?"¶‹-JYù??Z³Ö?v÷ê¾Âvq?Y¯Ïì?Q(º5|ØÓ?ˆ©¶9Ùý?uB
¬õÊ?ï>‰uÓ[?up"ëI¯Š?o·Ùâ.?V‹rg^[?"L‡2²Ük?tÙ·Û:ÜAGN4FGL J2117.9+3729?×DÚwQ½"À ŒFŸ¸À9žY …F%À;Ù ™hr@}xåÄëW@8J"xÈi?±«HÓ=?¿Téf`‡)?ûMÄ(¹\®?ñî¹Ç—¹?ßèGœÌ©ç¿áJ™¶õÊó¿àÙ๨¿åÉ£ý˝M¿íǍþZäR¿Ã·¹Õ¤6×UNASNone3FGL J2117.6+3725?â"ˆÎVv?›Žùâ?Ÿ¼-‡š? yÚ8O¦?Øæ1+Šâ?Â|3	ö+ž?ÜZ{ ²¨?ÉB^'[?·âÅÎÛ?µ/c!MÝ¢?Ýõô%"Æ¡?Æ­Ã$!%?韗»Ú}?¨þdFìò‰?«°2ŽýÇ?™ '°l?¡µaÂ?¤¬G¼Å'C?宆¢éE÷?£b.Úo2ú?¾Ý™Û€;F?˜-³òF¯?É׆šÊ'?œs"æöEv?׵y?À~‡¯â0a?²䞻ò~?«óÑË«?â2htªï$?Âþ%VÉ?ÍË0=hÿ?ÆمŠ÷rñ?ÁIª‡ÂE?Á4ül—?äL!†xN?ȈPF‹?äܶœ+;º?°µ«*Ò?µǓIË?¡¯ã»2ƒ?ÐñRTØì¸?®AS¸ ?Ü='ã°Ð(?­¸=!2P?Èýxf»?¨ÊڥťP?×Cú'üz?ª4‡MIXED4FGL J2118.3+4055¿ê\	'âÀÁ)/»¯À;-î@ºÛ3À<j¦'F•ç@"OÄÄÂZ?÷eâ}8:?Ӟ)`ÌsŒ?Ó|]ž–¯?þm‹ÕÓÝ@úÐ<BüT¿î‰
€6œ¿ïÿý¡UûŠ?ïÅ!ò6?ïÿ"ÕåzC¿Ú×ÄØ6¸¿å[ח+*PUNASNone?슦"–äø?¹J"•õw?a¥0.¦›ˆ?['@MTG?»¡â¤‹¡?¹;÷k˙á?êv>R²;?ıžž?a,°â\hM?w8
>m?ÅáD€ž²?ÃÓ1ÉYXj?êL.0·OY?¬°ž¥¿d&?³÷3í´?~ßYoœø?ÅѧƒxV9?¬S1ò?î|*l1¤?—a2AI?MõW!ž‡?D–ol
?§Ê݇¥¾P?—Rþ¨+E?èþÜÑt?Ä}•üoìf?wuóRF?ž}÷9£]ê?ËJWù!zµ?Ä/z‰'—?ãë0šÁ¸?Ì«³uko˜?kàÏ]ª»å?"þ¡üU?×ñÞ8Hàˆ?ÌxYK(zü?æ$aê^`¼?´äqÝà?‡ÜÔÈ<ò?Ô@Hî?Òþ½Dïs@?´®×À?ìZ'·¶ ?±æiƒ‹Â?f~^'ó?p†¾Dy¤­?¼vóß,Ã$?²½»c¹AGN4FGL J2120.0+5257?ïùÒg҈_@[©ßaúÇÀ9?踻ÐÀ:àF3À÷¬@SN×(›U@äõ$ÚªÜ?ÆF—i¾?艀qÕZ@"·þ®û?ö?ÊÎDò?ï}{áwÔ£¿×ïÈdÞ&¿áÅòÞ.t¿êûÒï)¿æÄþ;â¿ïÿùµc#¼UNASNone?Ù'D«U¯?Æ	YÿêuC?"1lWÃÀ?'9`<ä^z?âÊêúµ=d?Æ›7(‹:?Ýkäõ¯ç?Èø‡âHEO?´ÂÇ'àÐ?«~·:ö=b?Ýd5P¼'…?ǑÕ'í¸]?ژgzË?´Ø6JZe?¶N+U²þ´?£Aó¼çÊ?ßÔ
¯|@)?³«T°Þ&?ÐaX†¯?¦p²_W6D?»è'e¾—?–¼ôMÖ]Ö?äRA®ÿö?ªZ40Å?Ðr»ÝýÛ?ÀWÕ\›êà?šoŸCSq)?"ƒå`&~?æó%«\)?ÀÿÆOÁD•?Çðé"
¸?ÄcGJõÐ/?À®;ôð#á?½;×~xù2?åØ6¡Áu?ÇíÈ9W?Ò~Kԃ"8?¯"q³'?¸-@ðíÔ?¡Äürì?ã»1÷@`:?±l)0n+?¹êhq·?œ°"C)±?Á±¼S?¤a$"°±?è{F¬Ú
š?«WŠ×9+SMIXED4FGL J2120.5-0138?ïà"JäÀ@¾&ÉÀ;9'ôcê‹À<ž3>íÂ@!ÞdNß?þh7‹‡ˆ?Çh1ôo¿‰Û—.ʹ?ÃfýNÉ@$`Ρä¿îâÅÝo\Y?îY¨¿ãVöâv¿ÞVé†@÷A¿ÓÜ:¾l⬿ÌQü)ÝUNASNone?ï㛧ª˜3?`½ú3¦¸I?+"œ´§Öí?´Î_¾;m?j«H c?`E«Ã®9;?ïшXÿv?sé˜ÄäI?@¥QÆÓL?K0C&'?udyÞi?q
‰ª?ï~Ú	»?t·†ëÊDƒ?Y}ºNpª{?V·èÌÁ•?ÆEaB—?rä>¸m8?ï™G@Ó§)?g¥·óÕ°?M'J›Ôº1?6ÏÀ–F@?‡Õ&¬O?gŠŸÃ¹¯?ï˃Ý"c
?om#­ åt?<Q­?©÷?0àk¦¥æ?xxö©Ç'ˆ?nyçA¬?ïnÇê1Y?ê8ŸWz?Q)*j:?`c'*Bö?'*tWF·?Žjtw}
h?ïã"bÈÍ?ƒtoÍE(5?]57?P
vç@Q?š°=Yƒ¨6?'ôwþ§Ö?îáEÆx§?"Òæݾ8j?a*P7²=9?U?õðNàw? Øþû	=?"ÙiB'¿4AGN4FGL J2121.8-3412¿Ýg–ÀFp(€QÉ÷À;É%,à2ÛÀ=*"¬ÊÎÆ@ £~‰x?ü—£U>S?Ú¥‹-lË?ïþáQ¿u@#È\$Ä?ý=ÓLKˆ?ï=è΋î¿ïÿõƒ¥;Ž?ïþìɹ¿Ãbý±@¿é3çcQ¿ïî´³ÑSDUNASNone?ç'þ,ˆ¨?Èí›Î?§5çc>"?¨?Ž
oE?Ëõ:,ÛÖ?Çgõ½[ëŽ?éÒ£²2}è?ȼ2]ÿ?»hÚÇH?Áýnb*¹ß?µÍyï$þw?µW\7'[?è–Ä
Œé?²Íâ1Ê?²»,¶—V?¤Þ|_'…Ö?ÄGa?­ao?®Û°ˆ™!?沍0¥?±{ëæp÷_?±AÑlÖ?®ã)\O?Å‰l"˜?©R±õþ@Û?ãÂØëû!…?Ëîɽ´è?´¦¤üÿH?³—ûmà?ÓP¥"Ӄd?ËoB~»Øð?ãÆÕe]ãò?ѝÅY{?Ë}â=EŒ?Íâ«ür¬Æ?ÅfÈ-x*«?Ál£+é'Ö?æ;X'çÀ?µ©€0ÃÀ?ºD+NÉwê?¬K_ Šµ·?ÉñÈøµf‡?³Ä"ú:?ÙÃ<Áe?¾&#(	?Ïpô8:rÜ?Áàø	ÞÈo?քn§Ü-?¿É·]hª¨AGN4FGL J2122.3+7653?Ýöb-­Éc@2²IÂÁ±À:ù» Tž¾À<{:r•@0Fþl,#@£a~ ?Ëüð@šNö?Æô·7_?úk©f–7@ôÿý²¿ïÊ,¿%Å7?ïü% "Ÿ½¿ã[Š4¡È<¿ä®‹™%Ö¿ãÁöD•[F¿å™Ž´/óUNASNone?ïv`å%«?¯Ú£èž?_‹ñóEZ?a)µ¦U˜?ŽvH|]®
?¯|å)Ñ:?ï´ð§iÞ7?|4{ò?Z",Ye§?`,$w‹Ù9?~â§,Îõ?wlâ""À?ïRS,€o/?'QQ™Gý?jjdDž³.?f"u³þ?'hMÖ©mÃ?€¥~Þ¼M?ß?s°SGåB?~fœ	=ò?^5hOÉ8½?"•\Ѫ<?r•äÈ´ì´?ïÑø£ô?"Ú{ˆ¢Ö?pó÷ªº1ù?f¢Æ‰©Æê?˜èÃÈ?"ð3‰õ?ï^ÚÖв?"éyÿÀ?sSs^¸B_?{/Ú׳õ?—?Gʌ.6?'BºŸ)¤µ?õ2?'î46φ!?|DZǝï?wgœ(å†h?£}¶D??p͘ZÇz?í†Ùe5?U"î$"p?'‰83´I?|³Âï72­?®1+>n»û?O%8;SAGN4FGL J2123.5-8315?Óñ¸™äîÀ?$-òˆHÀ:ÍF«µûÐÀ<7™èsò@@ûEاK‰@¼Þ…[ôó?¬DµÝr¿£îî¾AÍ3?á3W{V@¾'$Ý¿ïýýÇ@›Ò?ïºa¤µ¬¿çÅä Óõ‹¿ãÝ}‰˜š–¿àì1¡¸¡ó¿à·Ð]óÑUNASNone?ïÉ\EâH›?lm¼?£©?HË쏒¢z?<¢L›ÃØù?x8_wöºê?j¤¦l؜Â?ïÐ{žd&?sYKø[XÝ??Ž$·.K?F%wÊÆ ?uÉN"c?qÜ–^Ú?ï8è±Ú®?‡\H•æ?jζ ªHØ?lÝ ·tÁ?•‰ö˜F_?…V³¬D‹?ïvô;6ô?iÓԥ̔V?ZMëÍif?B&I†?3Em@¡æ?iRtú¥c?ïŠíòa[æ?¨äqûa2?]¿ú\Í?SÅGYõ+ž?‰Œ"$•Ë)?€_ˆo|º?ïbXxù?'_¸XhÐ8?Sgòùviå?déejƒ"ª?'†^ƍW<?«ãqt¤|?î[\g_	Ñ?•xϏ:t?y$ÛBºœj?vúì7#ÂM?§%ž"©óæ?"ëÿsçN?îtÚFv˨?‡×;Õ]ÿ?rœkqmI'?bî×»G§$?¦^Î*eœL?‡W+1aAGN4FGL J2124.9-2433?ÙÚÿ1›OõÀEå.rÚ0À;sjZç­À<‰M DC&@‹/ûh@Eˆãhð"?ÒÞbKy¦?ž‡ô¼¼²?Å8L7;*£?ûB"°Ìf ?Ë<*'ÆÃs¿êÍø{§@K¿×úÉ?#¬X¿æYlÀd¿ïýñg¶È¿ïæÿ8mUNASNone?ï¹d
ý›2?{YV],Êo?J®³Æuê'?@Yûûçß?ø$õ4×?z‰J&I×Ä?ïæãW~?'çÃH>³?a?ÀûTiû?d@êËÏB'?‡vVöOõ?sÆ*Z?îâlò»È?'›êÜÌ,?'†Ï¨Ï`‰?'øLo~ÄÕ?šnùè Ö³?ŒýÝÇä<?ï»KE"Ê?uûÆr[5]?sÔÃb×?X—:½â?˜¦¡h:¾ý?scVq'ȧ?îûx×W?W?—}nžKãŒ?^½g#W¢?Sòn§:ˆ?ž¯i>ÑÚ¥?—:+¡£¼#?îÑc›
•?xxW4?q"Æo+Ú?|œkS0¹¼? ¹-~Uë?™ŒÛé7v?îd$ѵX¬?•ê…·'èu?"ƒŠW•Ü?"þ(ÕÛ@?¤œÐJy®"?'x/1^m?íκ>;
S?'qÁB½Û;?€—Ç"Ç,ƒ?s"xt†;Ð?®îj9+[(?',ϯÏ=AGN4FGL J2125.6+0458?×kò¬À>Ü@¿ã°>À;Në¯æâùÀ<˜%·I­É@ ü´fú`?ü‹Ë*5]°?Ñý6aé?½¬ ›$´?îƒÝo²@?þH%Ûܵ"¿ïÿúVrÓ\?ïþ½_ÇeÛ¿Ïe
gs¿Â%›¨±:¿ã3ÁˆK¿ÙZã¦XUNASNone?ïàÚqŒE"?l®À§5r­?'žÛ¯­<:?©[,‰­?m« žã@?lF6Æ¿°B?ïÀá	xW]?wkéÛ?õ?JT6úˆ£=?P¢	¡´±%?|Dôrvs´?tÝTíâ­õ?ï@
ÒÊpZ?ŒÏ!ˆ2`r?f© n	Eî?sãè/%s?•)–‰?ŠèFUí.?ï%KLJF?uÀm3ƒ;é?fúz€1è'?J^ìž	•l?œ\0َ=?tâƒLaÁ?ïÅ%#%?y½´[/ß=?8IŸ¾œ<r?14£O.6œ?{èÔyÆ=Ý?y`ø³óqƒ?ï1Ìå»?—.B]•?^?¤F Ô?i·…Èp?—âi;?–¸Túì
?ïÐç8³Ñ?Œ¢´¶°Ÿ¨?dq°"Ó~d?lÊC´©û?œw­#"%?‹8¬1Ti?í¿|H65Ø?ñäíCò?sœ?czrqÀlV?°Ó܌ЋÞ?‡ðØMgAGN4FGL J2129.1-0240?ì™o{VÀAðuöý!ÿÀ:«åüjIÀ<=²¢i@ƒÉeeà@ÝäÅ©?ÈTí˜oW?´˜|c'í…?æÞ|Ý¡0g@	j
fEj?ï°~¿å±ú´f¤¿èf££׿ïÿ¬óéqH?ïût_ÎFÊ¿ðUNASNone?ïõ+,ËÝ[?rˆê K%?,´ªj¡º$?PÄ%_8•?RJÅ<?mWL(]ÓV?ïµÂŸwT?ˆ
"`/<?WÆß)ö
ƒ?lV¥*Ì#?,øZëñ?ƒD
øªÁÍ?ÈÈu?šª(x";f?k\‰­c1?wÒèûÞ\?¤®ºÖÆÁ?š?´™üË*?ïò´ "±9?JZ&¤"Ì>ôoݽrê>õoûÓ"zƒ?ZEÿy™?J(ÏU]í€?ïò[ڜCB?^³°Q?0
èãm?6-
šÒû1?WEòòÌt?[êœ#›À?ï`)¦A¯?—Ë0ðÀ‡?[µ]£¶á?r-H¯®?'?yßâJ°?•a™È;ä?í~šÑ8R"?£W«ô¡8[?v#k:›½L?~ðÙ"êv?²¨òÃz•R?¢ê'TÙv(?ïÉwÔç':?r,þú"!å?F–½¬Oí?"k¦§g'?zÞû:­×½?r	ÆktnBAGN4FGL J2129.9+5833e?ÅûäIb–ð@U›¡±–À8¯Û$~eÀ:Òe횢®@ÒqdFPœ@)Ưc/?³Hª~CQä?·˜¤Òód@ÏPB7²õ?þk‰0?ãÆ¿"9C…³*¿ÝÐ&^
§]¿æµV¬µ¿æéìb"IÏ¿äÒìnºÉ?³õR'AUNASNone3FGL J2125.8+5832?ÂÒ¦§/j?²ÓEXÙóÂ?¾£,ع?{ÏuÓԙn?ë[É¡Á~?³^XÍQ?à—êòŸÉ?Îñ–8nº?ÀW+ë–;–?¿Rі«ô?Ö¤"$öÀ¢?Ç
X–š?Ø´mµ»
]?µÕãÓ4×?±þé…ß
? W«—5 ?áf(Qò€?¶@ÊÂeӊ?âƤՕ{Û?²¥Ñj;>7?¬oO­_v?Š˜£f?ÖäÌqÌå»?²ï';‡Ð?·îÞp±@?ª^gƒÔw?†+yÇÄ?zôðø'#ç?ì©óƒgJ‰?«Þm™l•X?ÓbÅé?‰?ˎ¨ÞÊ¿ñ?ÆÐ&(]Â(?ÅÐ ¹wÊ?àš"I
2?ÊÏiùݕâ?҃ýÀà…f?³8"f½.?°ˆu¦Õ>?Ÿ¥fÓßë¬?ä¬òj§Nõ?³Õæõ?×»—ƒ-¶?·Et(ºÂ?¶Y¼î͍?žHÛæñN?áWF $?º]»	çñMIXED4FGL J2130.8+2649¿v±W°³ïÀ1¤÷‡‹zÀ:ƒcj2£ÁÀ<T^üå™@8²yŠ@5!¬ˆŠ?ÖëU£öiÔ?Üýi¸*~Y@¢0[è^#?údW†¤Ÿ?îpï ´«n?ى+¶c¿æ˜ZRp¿íßø="ßE¿ÑƳãÇ»¿ïÕå¯ò¡sUNASNone?í8"K??´5ål{?…™¢Güæ?'ñŸtaí)?´
È5,ji?³#̬a4ˆ?îˆÊqÉ¥?¤®ž(=™?'¢ ãÁ¯-?—EÎd~9?œDï¼ê@?š&Ž8œ¼?ì'1´¼?¤gÀ•:Ø?¢|…Ö?"EÈ9©¿¹?¶Õ¸3n´—?¡"q¬ä?éñü÷âÐ? $ú"âþñ?¥Rv¬p'?'+KÐft?ÂãnuµP?™ýL0* W?ê ·Ö©O?½ƒyǗ-Ú?"­³éY¼?""MÔ¶}?Äçj)`îÐ?¼P,h=Öû?êÆ÷%:÷ù?Àòõ,´¶M?´jêå©¢?¸á­)è]?µ][ð~ž:?³2s"Vó?éj1I¾?­pôr£Î‹?°Ýr^Ã?ŸM
ò7ň?ÃÃhüT
*?¨¬.Ä$í?â¨dÚínO?°s®c\?²Y¬™¦…?¦&'}E?Ö/Þþ¹À?­ÈÞO²îöAGN4FGL J2131.4-1124¿ëîüú‰jðÀDN#c²WÀ:½T#mÃRÀ<aUy¯‡@cD¢œL§@¬Š7&?ÔÃmãæo?Û(mÀÍ»@9?l&™È?ûëg\…'û¿è…–½q:*¿Á¢Ú›¦º¿åÕ<Kv¿ëÙB[Å"´¿ïÿùJYQ?ïÿÚ@RÖgUNASNone?îSnFڄñ?¡*¿‰QÔ²?uʬ'–ÚE?o¥´v˜i?¨Æ0У? "'q)?îb¡]2`%?§gŒÑ&´?æΰƔ¡?—•ŸŠŒp?¡b'Ð+0m?ðèBƏv?ëe'ÞŽŽ?¨Qp'½›ý?©'D_–.?œy%ÔҊ?¸DI၁ù?¢§}|»9?íqÛ8,r?"ñnô}¶|?"yð«?w×F{w7?°L$›À»G?'R6X¬"s?ì§õ§â]?¯k—uúnv?…MLªv¸?'í`Ùp1‰?·HV©™'Ã?®†èfˆø?êó³õv W?¿·þãlÄ?¨ÓÙ]3IÊ?°^!)§ô?»øs¦?f?¶§UƐZœ?éè"QMqð?­vðBåÜ'?ªåÏøÝ>8?œÒqòù—?Á¤>½nÏ°?©';ÚÖä?é Únݨ?­‡xoRs??Ÿ¡óKò?'KøÐ+"?Ljse—"`?«~®Í+™AGN4FGL J2131.6-3714?ïðÌÓµ,ÀG…WÞ
fñÀ;}ÁÅìßÀ<±ËY/F?@!B4éì˜?ÿ "•MÚ~?ÇB$½¤Ä¿¥µË\??âyÆ?"ë_@É͓ò?âh®_ybB¿âoçïhH¿äþîÝî³'¿â¥w=¤%d¿ïáÜÿI÷›?ïÀ­TžéUNASNone?ïçÕE†
à?`Šþ±VeÇ?90Ácñ@?;Š$?%3?e¢¨Ó{?^Xì"yå?õ÷h'?†üF%íê?`¨BgxF"?k%cܲ>Ê?…rqâpx
?'™LœÚ¤x?îßZþ¢?"Kq'3å?wÁ¥Hƺ±?(D["hl?ž$SîÕæE?'…z斜?ï/9;émË?"aû¢j$?`[ã&\?N"Ä6õ?˜
w­x®?"1B8ý×?ïË¢»VWÐ?tQ!ÑþO?KJ]Çò??F·ó)‹rB?vÅVªl\?sc°»™?ï"H̙î?š¯­?.b@?gìý[@[¥?xl¬Sk!?šž5Y[Ä?—Ò¹³°ë?îj*CÑÞ?—€Ü…è¼á?zñ]hL'Ø?c}"Žò?¥ÿ+J¯ÇF?•‡<?ŽoÌ?ìç"þ÷Žº?¤²Ì^|‡ò?z¾Uñ?vÖè ñ?·G;ûD4?¤óYd±k¯AGN4FGL J2133.1-6432¿ÛìØn|ÇÀD¤øßzN{À:Œv›gÐÀ<‡Tn^@tG]â‰?þ¡ú@£^>?ÀV9ˆý?äê^x[[p@r)AAé¯@0ì1A?ïü\ý†þâ¿Æ"œY½`ž¿ÕD«@5$O¿çŒ |aû¿ï"®"g³î¿ïÿÔÌuŽøUNASNone3FGL J2133.0-6433?°Æ¤¡ôD?µ—8ÕÒ?í­óå$?ºã;à<&ˆ?›¯'Âe? Àê"Wbô?²HÉXµ4?°x}ù>À'?ꩧʏ'?·Ǜìwe?¸iøU"¹?°©×$JªL?»¡ƒ!KîÛ?¦ù.RïSD?è~»Ôã ?°®
l$?À4Oîz?¨$ôú>?ÊÊðK#ŒD?¤+ù€f‡?俛_Ü"o?«ªÍa†Óz?Â6¢5kê?Ÿ«v"¨G?™Uýø
Ï>?› –ˆÏI?î''·wH?§$Ó©GÒ÷?"ˆ'«ÛÝÙ?–¥#\[¼?¦©¢¥VÈ+?¨,í
Ô?ëT]œµ¥5?¸¾Iœ*?ºAÇ9~Á?´yÊhMÚ?©"þ1C+?›è.ƒõ8>?êÝâ»ÃÝ\?¯‹%Ò;e?¼Fë0²?©s–î³@?²£©—øy?–tMè?è*µz¨©?®¾N">(?ÆUçTŸ?¨¦‡|PSR4FGL J2138.9-0408?ë©¡F»ÀC\ó^1
¿À;VÏj5þÀÀ<¬àŸèh4@Š ¹ˆø7?úC(ùôMD?Ý3ۀnÐ?æÁqðdx@Kݞ¬(@]wõ#¿ïÑ
ŸYƒ¿ã•Ð-hï?ïïñʳ¿Ö@›Ñ'>3¿ïü–ä•¿ðUNASNone?ïÝi'^Y?l—až&?[q½Ëê²?W¹°îiü?dÞ
ž©Í¾?d\	Žr?ïTÍ}²ïg?ŸQ©ùŠ±O?qq¤çð†?Wr:ْ|?'
	  ø?š©æ½7?íë3ƒ1W? Gœg2I?'¬å
ÑÈâ?²eÆÂí\?¨vQÏí$?œmþPÌwó?î­Åê5ú?†BhóC?p¡"}ˆU÷?a\5כ'z?£§?…µléY[?ï°õ~?}ݼR9o?rA"r?n_ˆŸ³{?uDcOC,?t2ÅIª©Æ?î*
®7i?²ÑW,–ô¿?ˆ"O…yQ%?¢ËË6rù_?§>A9sM±?©ÑÇʎÁë?íuÐ^;?¤ôßþl}?'
•1-‰ ?¢
¥«?²àì1Ÿ'à?£!CŠ'ö ?í^‡ƒRÁ?Ÿ!˞?s9êEzPÞ?rY'"Y<?³Ø%@bbú?ž"°)<µAGN4FGL J2141.4+0733?嘆˜vUÀ@6*Ã") À:…ì燫À<4ÛE5"7@kTù‹±@:aàŨ?Ãóʨku?°‡D­Y?ä¬é¢Æi?ú|=•âªÛ?ïÿtõubƒ¿Ûh(]lAÈ¿çì;AõmÖ¿æL,ÿ<Œ¿ïÿõEq#?ïÿµøtñDUNASNone?ï«Ô
Èu?†8Øoµrþ?RM‡§9¤k?TmEeSX¥?'ïZÕ
/?…è渔?ï:Úwì[ï?'ÑSÛyÚ?w?$˜¼«?}JŽ¸wÒ¶?'ÔçÖñòT?Šg•,ÐØ?îJ"¿·?˜àVkW?…êIÉó_¦?"¢_*éÖ?¥ãK°«Ï"?•ÊŒ£zš?î"šj\?"Ç̔7?ˆ	«ò¯?oDž"#? ÍÓõ|?är*sØ?ï^f'‹û?–
—ïÕ£Q?`™b==s?cM`uքÓ?' Þô?"ê˜B_(¸?í¡7šöæÒ?¬'uäÔBœ?ŽY{7k?–"ÅZ£Ë³?®V'Š¸‰?¦b÷B­~È?íkÄJáêZ?,y	öÓ?€Ò¨wæ"?‰2´ƒ
ÿ?°¨ýå?™ &Ç,3l?뜄™h'‡?¡@U,B®D?¢J4Úó?<…7$?¹öÀø>{Í?›E'ˆØÕAGN4FGL J2142.5-2029?îNJ,-`ÀGEŒÒ
ú/À;oA×:åÀ<ŸÒcÃ@ ´í6y¹ª?þñ#Xʜq?ÃN	M[¨¿'á´+ì?Ë2að
?ù\ò3Ž£¿ïÿÒþÀù?ïÿüÚ±'Þ¿áL	Þ¦%¿åÁ(ôëÏÇ¿Ëì쥿Ëiº¸M9UNASNone3FGL J2142.6-2029?ïÝý×Ó¢?iµP'¸X²?7öâ/…þ?1ßÙ
_k?o
'€Šo?hlŒ¨ÂD?ï'IN†)?y±µŠ]?Lc"Vœl‹?V$xFÓ?{2jê9Y:?v$tÓtœ?îé´.ùÆ3?'gÀI)ìB?s?MÄ>=ê?Op)û}?ù¦µæö'?Ùóží?ïU]£Ã6?sœÑþ¬7?_õC5Ï7¾?LV#pó9?"U	QrÛ?sgq‡Žu•?ïÀ·?wbñP2	?MæéÇñÿ?Fö³Ë?|4˜âß8­?v'Q¢DC?ïSÙŠ©ð?' Üà?\óÒn¦©?lõêtrٔ?"µ n§Ö?FŠ«ò?î›<†Ý;?"¼Ojæº?n±jTâLg?r¼Ò"‡X?¤a("Ó?":aFÿæ?î/ôD5*?'QC¬Œ—Q?r>MRw&?ih=²ç>*?ª°"ö¶bû?'QÔÖRÿÏAGN4FGL J2143.4+6608c?Ê·ÚËΖ@#¿;ÉêpÀ:üíüÈ=À;¾X0ë@ÀU9@Þ~bÜn+?ÂÌv¦$—d?¹ŠÔø³?ödˆu"ç[@É2Vˆ?åguZ0G¿á~¸+¿ä߯þ_ìпêDùdŒW¿çE˜%%Sw¿ÅaŽ:jßóUNASNone ?ê<9ג"­?ÆiHç>W?fêEÀïA?e›þbkæö?ƳoŠÄñ?Æm§ßhÁò?ëï€ã·—S?µ×°™çýh?Ž·"j\?ŠœÐ¢ÿ¦?¼­âÀT?´jh8?ìŒvç¤$É?¡pBª–äU?‰ûð:Š÷?'ä—Ëäq'?·«	Di"Ù?Ÿx²ÆX˜?ì®aà£Kþ?…ĸnUz?n,ªï1›?hÞj8jñ	?¶Ÿ+d«Òá?"LÁ_ßf?èV
~'³û?¿Ä³Va¿?ÀžLNÂ?rj=/fB%?Í©Ñ…6?¿ÅNÿ¡?æ9OGn‡%?ƖWKQž??¡òd…'?£)TJ>?Ñiƒ$?Øç?Ŗõ(ÐGš?æ¿h
 N?±w—·€?§UÃ\ãš?˜ªh0Üdò?Ï,îôG˜¤?®à!u=N?æ˜ØNJvD?ÑS—{?¥òÐË ?ŠBî€ëf°?Ð7rªd?œT2Í«Æ¢AGN4FGL J2144.2+7709c?ïýX]'P@2.bÀ;y⏬°ÎÀ=6.Ú²@ #apˆSK@7#û‡Ë;?Õs4?¢­??ïþÑa‡•@òS—VÉ:?÷՜NÕ¦¿ïÿÿ&¦³?ï芘tÖl?ïÿ§ B€-¿Ô:©´™Ð ¿ï€]óÑ"?Ý+%þAcøUNASNone ?¿<ŸSÔ?Å_ù^
o?Ô՝Vù!?ÐJ…Æd9!?àåmDÑì?Ó•«U?ÇIIþѓ?ȉWñÈH?ç_ka>Ï?ËW¨¶åQ?¶rÑâÖç?µp"ì¹?٢΁WÙ[?³ÓàÑâAp?Ö®Â%)[?³ï)µY^X?Ï\Þ²þD"?²@E7gt?ØÈ`-´?¹Yèù;0?âMÊZ¤?»«ðý6T®?©˜!ëÕT?—º¶œJ(6?Àø
öÁEŽ?Áö‹•¨|?Úiî)?Р*ô²?݁Sk?ъ0
A ?»o´²"h?Å
¥j³'4?é˜ìjÌҁ?Ëõ§èÍðu?·Èç÷ì?»ðÿ O?Õ$t¼Èü;?¶}wi´s?Ùן9ÒÅÆ?¹"\€Ïí??Ñì	d=þ?´êfˆÛm?ƱQž?¹â¢þÆe?ç¿ä0Ž	»?À"üŠ]ö?´Èél?ªÓ90IàMIXED4FGL J2144.8-1600?ï&)lWcŒÀF¾÷øËÀ;u¬QéØÀ<µ
qs	ã@ ¡¦a(9?ùú¡¡¥×•?ß;m>qÕ°?ÔrcÞ=?ø™&âÂØW?ûZ$¬1̬¿êï<-­¸5¿ë†®Š©<¿×¯•¤—y"¿ç°¹`´JË?ÍYjªmÒ@¿ïÿþR€ÖTUNASNone?ï—t?ºL?‹ß»÷Cl?Rî@"9i
?V²üÌ?‡Å(tÓ?‰n&è ^?ïŠI)4?áyb"§?c•K®5§<?pvìįŠ?ˆ"ÚÎÿ=I?Gý3‹·s?îÓDFg)?ዃ}å?x²Ìw
½?`,Üq z?«$Ÿˆ=
?›#šSX?îÙæö;'–?…·Ê¿-H?@ò^VRG?7};&ë?¢!4Òu?…št_ù9è?îãYG*G8?¢ê0KQ?i¢ÿäœ5L?i¢¦µð=? 0;«·²?¡xZámã?îÜ"":?¢Ê$
"Ñ?pƲT-À?'Ó¶Õâ¿? %xAI´? Y"Ò׿?íØ÷f8?£ ê5‡Y"?…0l»\ep?"þE¾ñ¯ë?µ;*¯Z–?¢ˆIY±?ì"ÜNR¦ô?£éSÕºé?HÚÈSv?R!ì,š-	?»1Öþ:>?£ÙmI×AGN4FGL J2146.8+4808?ï|¹JJ7À}	@¢CÀ:oD"n¿ÑÀ;È[ז@FE}@¥1Àll:?Ç7ׇ»Ëž¿…ðYfE%Æ?ÁÊTâÛVþ@#J|ù{¿ØɁÿ-½¿Ü@ŸWs¯¿í±VNÁ¿¬Æ¡~Y;¿ì­×^v-?°žª`Í[yUNASNone?ßnµÝ>g?Êè‰M¾q7?z¾¡¾•?x'䗏\?à	¯"Õ?Ë:èo{Ê?ë9""<?·/ͶÍI.?]ÕþÚ¨?esù¦…?Ãkoxz?·q±´r­?çá\?,Kõ?°"5Õ¹€?™Xvžà?Ž&"Á¢p?ÍO‹Öî?¯lÓ˖,W?îÆÃWqð¢?ƒh†`±H?eæÇ#?'?Qg€)t…E?¢5^†{ê?'°)‡œ™º?Ù»o'Cè?ÈÏ<ÈïY?LVæXÉw?…¢ÕúÓû?ãpìÀ÷Æ?ÉÔ¹,v?äO¬!þÏÌ?Æ×oó­â&?iæMq¸Ø?€;/Ö-Zî?×,Û!ƛ¨?Æ­ò{ªh?á4Z¶Á?¶ÌÃHr?¥ØôJÎë?–/	¿:?Û4xÉ{š¼?µíéâc5O?ìpñÎ? Â$=ù•?'뇌¡›?t5aŽæ?º<#Ï_? @1ymÖÒMIXED4FGL J2147.4-3854¿êPêõñxÀI\лnÖÀ;Ij­À<†,9
ä@!ÅX^è@ÈÈ@vÕ?Çãr€¦´¿Ÿåg}+"?ÕXTßd@IqŸŒ¨¿Þ¯¸¿ÏŽH¿ÞØs/Àã¿å!wI¹L¿ìŸÜßi‡ƒ?ÑÜ*7áïýeá±5mUNASNone?滑Ág¶??ö?*š?GJÒð&?A¸'èQŽ?…j"¶Ù-?~×ÞFœo€?ï±9MÔt6?"¿}ÉgB?T¿GÔW(?a}Ö³ó?ÍðV\?»7w[CW?ï+ƒçUº?‰uAÚò¨Ÿ?roù°'?v´¡O?™>':ns£?†uC¢6ä'?ïÅ]׊¦?añ™'‰Qè?!ƒ˜€àÕ3?'òêAtŽ?|Ä÷§}@?a¤¤=x8?ï‰< º?–ð'n#·$?\¤V"Œœ?V]¥…´­?œ–æ×}?–[!†.û
?ï?w(«? mJî&=ö?\pYXïÚ?oVb@F¬	?–W>IIœ˜?Ÿjn ×'?îUC€¹–?"ÑI‡~&0?Þ 
ÃäN?€7²mS×?¦¯ó÷SÌ?'œ´‡r?ï0Ž›8Ö
?ƒÂ$¶™]Í?<ù!ÇBë?;¢Î6¶x?™}´¯Ì@H?ƒÛ×´äAGN4FGL J2147.4-3713?ïÎô9£9ÖÀIðEwÙUÀ;=£_9MÀ<¥°<«'@Jô	Q¸Y@
© öÍ?ÔiÜÓ3?Ç(xY­ñ??ñÅÓé÷ÿ@)T ?ïK¤C@Çp¿á`<ZX¿ß£™!пå¸Úýgr¿ä°?bì^c¿ïÿþó…õUNASNone?ïå¢+c†?X¾Xçd?AN5#Q;2?3½­P)'?f
G6__y?U,«®"׆?ï²öýh(?{?RÚz*Û?TjŠ³X?XÁ;ÄÞ3*?€´ïlÔ#Œ?wQ]‰«·j?ïdTÛÏt?|(=,¤'?gŽJì/?h
p‰~?ƒ'}7ç?xѬK]z?ïcp¨0Ù?lp
gT¨o?ZHCq_
?@c'Ši4?'è)¤³?k–µ÷cÈS?ïÊ~	ßì~?i`k'{Ò?Pº˜³)?DÖ53ˆp?v'yFÂL
?fãCv—J?ï?ؓÄ1?"ìp"Ÿ3¯?aÜÈó–"?n–á~œ&?•âYpú?'Y¹&I7N?îÿnLäµ!?‡bäBÓ\?rՔæ¼@?qŠfQâ?›\Ñ,ÑñÚ?"¾%¤†/û?îdSÚó?‰zñÜÓ_v?eÒHúª1–?Xüï.Ø?¨aæ6ÀÐ?‰V9Ñ°*AGN4FGL J2151.2-4034?ÞÑü=ÀI^xB0üøÀ:ó'÷¾èÞÀ<£›€#¦Î@Ö7"¦˜?ýŽ]%u?à.ªØ†>s?ÊÖ¬Š2é?óŽR
}?üɇ5=úb¿é¹j"Ù5?ÑJ?f9¿æ(C ¾¦ï¿Ò<Š?3œ¿ìòs_ž <¿ïîövÛUNASNone?ï|!¥AC?†ˆ9:'^Ÿ?cË^MO?Wz™(y~™?ŒàRul?"ÉÈÎtôr?ï´,µô ×?€+«z¥·,?WK]Æä'?`ì(Û?€ÉÀÍ´?zr|™`".?îú¶xˆ¹?»Âê?|?W8?zíO…@Ÿ—?™™[)s F?yìníb]?ïÕjDW?u­ó¥C?p"ƒ'/Ku?]Câl—?˜\±ô¾µ0?sþÃ~=G\?ïÀÅá?"¹¾¡=?rßÍê0ñ?fx¥ðub?™FÑ ©?'áŽB%þè?ï Ìf™£?™b$'zy??h·9iqH?u,}s£³?˜Ï'<Ëb?–󅛧!?óÌÀã?•ø®£°¹?xùFÃç?#=Ó§?¢¦Bp#9Ò?"è}ü[æ?î_ÁOQ]&?')öí‰e,?pDt_¶'}?qFNé©Á?§û\z{Ýv?@ÂÔ*®AGN4FGL J2152.0+4718c?ïþƒ7(òÀF¶¿DNÀ9®	SeØ¢À;À*zýÍ @öê5hl¦@
Þp?Á—ZúøY?Àˆb½Þ?ùÅށ*7@ՐÒÇñ?ík»9ýR¿Ý]Õ¾bü¥¿å {jÚin¿è>25r
¿è$SN[®¿âþ_
UNASNone ?롔
ØIœ?´=Àüü?qÆ
ÉZ?gÒÒNr{?ÀëwPæÅ?´/D큏?稰é"|?¿×ûêNJ?'¹ÓªpY??€Ì†§^´,?Ðϐ‡³N?¿SSy¤±¦?ëuŠY›ãÝ?¤_0Ma?˜7Ñl]?Œk'Ÿ"?¾E¸Ø	}?¡³kz=?온çP—Ù?Š°-‹§´'?šŸëJïÅÿ?s<Ì­ÂÄ?´'½ñ¹?†,Ö·W%É?æ3¶ÄÞÒð?¿Õ—þ]$?Œ1,?†çÍ6ݕP?Ò·	õÑû?¿¨Fæ!?Ýë!àê)ï?Ǎ>U?'`4¦øt?—ò¯øe2Þ?àwmnå³E?Ç°Y›õ
ü?屝g7$b?±è£`ûj?ª"X9˜v0?˜OÑ{<Ÿ3?ÑJ:+•?¯nDVF3?çôIî-(? NíGv?®Ó܊ªÊa?Œº'G†k-?Èyá&Ð‡?›¼Ô?ŒWMIXED4FGL J2152.5-0607?éhóÆ`ÍÀEP|àP7À:ÎØÿ
6»À<Yÿu6@^X(`t@MYŸ®†'?Áí¤ž/€v¿»¾[T9"?ôáQ¿tè@ ÷TX?ïó×Ûôˆ¿é¾ÃŸ§z®¿é=²GæHŸ¿âçØVmÊß¿ïûDgõ?ïç!ý€É¿UNASNone?ïÆ"tng?—"tÜZeP?mýZÂñè?•½º[:é?k@!
Wàž?z&óé­u?ïŒ`¦R?ˆ'"ã>¶?f½òvwÿ?sa)ñ*!)?‡8'ÏéçÚ?'9ڐ³ƒ?î§Dب?•—‰Q«vï?xsëy
È?|TÛU"°?¢€J´¡`L?"Î皈 Ü?ï·ð®?fۄ+2?^™´:'u?LhŸBð?|÷¡P‹ø`?bîÐDàá€?ï€Ê—W8æ?—CíÀ×K?'u€¤nùw?2¦4Kzì?z¯³–ž@?Š™֕ÂW?îÇ 	#®ö?¢þî/Q?w+æ~ŸÑ@?Š–Ÿ"¹9|? ¨'Ÿõý?ž"Ë)џ?í½Àš0å?¡}IiÏ~?~õ€aòˆÓ?¹ÿ¨/Ì.?°"£(o¨?¡5´}ç?îéæœ	i?ŒÏ7É
™Ž?~ø æl•?u;ޝI?›F—±;?ˆ49Þ4AGN4FGL J2157.8+7142c¿ï{ ò‹@*˜Þ 3çŽÀ:)öi~HÛÀ;©Â@ÐO@š6ªŒ1@;7T*?Ñs&hI•u?á©ñÖq'=@	ÂzÊÒ?ç¨"õ^¢‰?Ñàu =)¿áx+ŠÈE¿ê7\Wï«¿éò6H'iI¿í"bøóœD¿ïðà<ì™UNASNone ?æõrsm"Š?ÏWÅ)Ö?¸zNò?ľìjލ?Çí¸ÌÝ
?džH›œ '?ÚÈS€Û‡¦?ÒV®Ò)Ǿ?ÙÔ‹sĦ?ÐäèߟYÄ?ÆÇWé‡(å?Â)¸¸:;?âf"u›Á?±egåFÃ?¾ãH†£êù?¥lÀJAôj?Ózóƒ?¯ž¡¯&n‹?ÄN$´X?œÕ'‰?Ú P†Äïx?¯b"ñtC?Û8§èM?¬üÉÊÑÚZ?ã	Âü¿XÆ?ÑŲ"Õ›?Às¢JSq}?Ć!Æèöé?Ѳ¨áW•¶?Ë¡Bá¸'Š?É?õ<
?Ëé$˜vë?â¡
âýÌÛ?Ñêݍ©G?Ì<ÅX9R?Ƴ ‹2E?Üúh>¶Q¿?²ã=y?ÇÅø—½?¬Å$¹}!¯?×"›²âc?±uª"•]?§''µâ–?ˆž~ e|ç?ÞtD@ÝÑé?¶Úl@Y²/?Þ¦Éhd·?¶Jôþ–´½MIXED4FGL J2159.6-4620?ï&Ò:'¡¸ÀI=žÇÀ:—õL¼À<rÙ	1µ@!)n'E?úN¿ÓÀ?Ãæ[L
?²ÓF¹wÛY?ðî¸Ê·H×@5Ä:, Å?ïç3€`°¿ëõðý®—¿†4›¾¶¿ÒÓ¿ÿ4¿Ý?R[§¿×–ž<–‰DUNASNone?ïÏ^qûE?u¡eÃÓ?07…1z*?Q@.³?wo½0"Mž?uQ\Är?ïÐ÷"0{É?s1€7i??Bä­~ ¥?J䂍(x¨?u'¨5tÉ.?q½¬CK?ï?ó:þ6Z?‡PåÊ´?Y	]!õBj?QsÝÁÀjñ?–qÎE۝?‡9æÞãÿ?ïN[çmž?o¬^ïß?P‰)VKd?3ãá"ñ}P?•;Köò'ã?o5€Ž/?ï£RÀõ±¦?ƒºq®Ø•å?Ay§ E?3$
®׎?†Èӊ?ƒ…÷§Ÿb?ï…mœTxÂ?‹²NF_?P]ͪ'\?[îÒséPx?Œ˜ß1Î]?‰‰M;Æ?îkœ64¢ý?—7§]½Ðz?ará|hþ?\?&õÏÝÉ?¨/à?—>¼¢^ï?î9n":è'?‰·›Ë±Š?` Æߣð/?O¼YÚ)‹q?«g
K–ä?‰~2AGN4FGL J2201.0-6928?åÁ;ýÁÀD†Š›ÏÔ¿À:"›¯ôOÀ<n¼‡k @ö×?–@Uن³U?ÂD²w$K?×p"[<Ò@1êÝY@t^ÅÞ)?ìh§¾öJu¿áþËí©¼'¿ßÂ^ß´[¿ãßbцoñ¿ïÿü¿ÙŸC¿ïÿà‡êUNASNone3FGL J2200.0-6930?äuï@B,?Â$P÷ê1â?Ñ»áLá…?ÁfÕj2×K?µaÇúJÌ?§ú¼Èh|%?êi¦+š¯ç?¼@÷RB©.?¸"lóe–F?³'‹»›³6?´a±Å?®qåÎ
?àڵʖ€y?µ‹ß‰_\(?ÓШgEg?³v»'—Ë?ÄóØ/å?©%;ÅH·?é=•Jªs?›‡¬kµ.?º"!àz~¡?"*,͐?»ƒ¡u0-Å?"ãû$Qƒ?àž‡1¸ð?ÃY¯Åf7S?×níÿ€?ÄPù·çbz?¾Âr‡º}?°fҐ^œ?ãà8[Tÿ%?Çgã5;÷?ʛˆwQ+?Ã×µ7s£€?Åã–{4²B?·–½'º[?Ø̄LLò?¹òû4¿$n?Ú~̱ƒ—?ºwRO‹·?Éi^¢^î?®>kÎЖ?༽.¸éÛ?«°Ɔ†?Î-w'2Çþ?ªÈ«Èù·?ÎߓµR?¦~ÿzÏMIXED4FGL J2203.3-5009?ïý%¬Ú5ÀIWÒòäÀ:©YÿOÖØÀ<j–gµò@êNÿ—z[@Ï8à^*?ΚÞ=7˜ô?×Õ¬$5¿U@Ê%£'·Õ@¯Lejh¿Þ/]›f£M¿ãØ®¸ϧ¿êu|N/7ü¿îCˆêí¿ïý¶CôK—?è"ËáëBUNASNone1FGL J2204.3-5017?ïÍTɨL‡?«Sæ
éâ,?Y8áÝzûç?"¼=¸'9?sb–îY"?¤ÛVÈ?ï^¬5}O?'Wý(E¢?tŽl…µo7?h ìâQ?Ž
¼Q
¦Ð?‰Ó4ú?íDçØÓ?¤ì¹Òú,d?¡ÚPŒî#?œMC>hýb?©×1÷E²?žKœ­í…÷?ï£Zìjï?h`›«×‡?j;@°bˊ?Rk›¾é³ƒ?€št¿ÖSc?c­ô'cì?ïÌ'·î³?Šž*øç?QŽ¸ê=³+?lÑãæ"æ?uˆuȗ¨?"rÃÅPÒa?îLrÂ?U*?ª§gZ²°?‰ÚH: ?š~¥ZG=?¤öhS¬?¢¬¨ã5/g?ìó;k2uk?¦F¸!Q²?œ\¨nÙ?˜
þmÇ?±O¼Pžk?¢†B×n{?î)±>z?{Û¹;ÚÓ?‡ÑWÆÇli?wǶð¼õû? 9ùÉÙH?ˆ™ÐPXë¦AGN4FGL J2205.0+0943?í
Ôã†^ÀA¯íúCþ]À;ÉvÖöò:À='õ`iÍ@ó{}"»@:a$Þ?Ûù©#Ð>Ç?ìlª]a/@RC;¾òï@ÞÄfKäZ?ïù"ù÷¨¿á'åÞÊm¿Îª9º`äq¿â'N
ˆ¿ð?î)‰¡ÑUNASNone?í0¨Ãœç?´(ÞË-äŠ?žÜUÛó"?¤!4B§ÅV?­‡HÖöR?°¤…oþÜ
?îz!8	?­–ÿõšï?™î©B8q§?£%U	}Ê_?¢á]¬-›?ž¨a§r?ê÷«®L·œ?©›é½ä˞?³†ÎÚ8Þ'?¢‰ÿÚ¬Žˆ?´»Ó±;£y?¡1†7ôó?íªÎvÐ
?"ç®@ìK?£‡ðFFä?‰¯'8Ù
Ã?¡Ë'ÁqF?‹78ó?ëº}Ò
EÌ?»<wâ\"?¬Ýlf·m?°ùÖßäñ?´(¢·Â§ï?µ¯nwiß?é&knZs?ÄvæÑ°·B?¸'â¥S?¾œWA¸æ?¾;Š§…·Ý?µPWÂïN?èt·Óҋº?²+2»Ú…I?»‹"5·Ðo?©QÿTŸÅ?Àg^•Ùèá?¨÷"nTÀx?è<:ZÍ?°¶Íº'—?ºý—šæ˧?¨¬—qLþž?ÁJÊmeÎ?¬õé%ÈçAGN4FGL J2205.8-8254c?ê[ÀçÖnÀ@+L`RPÀ:·ìj÷ÆÀ;ŸÌiiP@Y7žR@Ì}´'m?È.ªb?ªË¡~•\H?àV<'gMí?ø:*¨öü¿ëÿ!HO$+?¾™‹¬Æòî¿ì¨ X6¿ãÚ«'!ü¿ïþ/ ¬ˆ_¿àò«ÿ!Þ¢UNASNone0?ïÒM¦b;? %ý'±¨?i=S—\ ?kP÷T)?šÝ˜"?ž¼.©g–2?ïŠY,8?—vdòY4‹?ð&ýp‡À?…4]ûiàr?–2«!L?6H[¿?çg÷že8ò?°/´J5]y?¦o¬°(¥†?™?Ìôß\?ÌÄ6Xà—?­F'g6š?ìæ>ø'2c?•ï«L‰t?•¹_~B?yÀ€`Wð?³_¨h0ÄX?">Îk9+?ît5÷*:Þ?§¬ÖWýýM?ˆrÔ¦
"ô?ŠÀ'®x5â?¢Ÿëfl¥Ù?¤Â…sd"?í,ø[›Ý?´lüÕLO?—+Gd?0?¤^ÂɌÓ?²Æb[‡?®cb`So?äÿ80¼®?²T‡Ç®+¬?±¥r$[?¢:ÃËFdé?ј(†Ãn?°»)I@	?赫·Ã+?­A–û¿‹?«Óm}kl‰?–±I?TT?Æ4uÂ=Áp?ªZ?¤v:œAGN4FGL J2207.1+2222?©
qñO‡)À:‹…ƒb°À;EL¢pñÀ<¤«ë«µ%@!/A0vëD?üãÙßö?ÌÕl®ì?®4'$D"?äfwŸ@B{pcÀ?ïùß?>¬¿à;×|S7µ¿ß:â
¿ÚG_:":½¿ØA«0šÒ¿äؼßï¿@UNASNone?ïÊéÛ{fS?oœ8ƒ ?0£ÜÄý?"ÌU§ïd—?y€ÔƒQè?of´óá?ï³' ø•u?~«…*?R9ë#P?Z6Ltx$
?€ï†…üÀ?z´ÕßÃé?ïIÎTÙ?ƒãøªL¢w?Y]AñßMO?L<vTÚ#?•0i8ڐP?ƒ³Óú¢T?ï\š€Õ?r©²"«?Ma}a"#?2ùĨËùa?"±¥¼Ù?r©5ÁˆS?ïˆV!}\?ƒü"ê¦"#?AäĶ§W?5@9L?ŒÝ1Lñ?ƒ¶§†ÁŸ?ïIC¾¤H¨?'*RÄ0°?Zþ.ƒEü+?fâB=Oá?•'¥:«…Q?'6§Ò0>?îq@,žw-?•©×Kõ°?`'xþæoÌ?WišêÃ?§âå¤b=?•Šo+È5?íô5¡CÿV?'vR?aóoz>'?Rø™Ÿå?¯£¦·à¸?'Ÿà
lAGN4FGL J2208.4+6443e?ïdþûÚ<³@—Óºý—À8ꈟvRÀ:þNôYÚ@
¹Ø©Nî@ǝZï9ß?«z}þDN?Ê(dM1Œ@)'^aµ'@D¼(?ÏÝ5$Ïî¿ßi<x¬9¿ãjMT¿æ;5`4>¿ìŠþ_kö¿ïÿøsCÄ{UNASNone3FGL J2206.5+6451?ȤNJÞ?ÁúÒjVÇ?ÜaÌù˜\Ù?Î…"v3?×LâxY?ÇvP‰@—?ÇúÂ¥Ù?Änd{nz?àHGÑi®^?ÉOÁBnÔ8?Ór
£¶Ã?ŀ è"Ñ?ۿ˼fÍ?´—'4³w?Ù+™PÉq#?´ŸÉŒåý?Æ)5æ8P ?«hØëðÓ?Ԕ4'
(D?§¬•IÓ³œ?Ò§¼uDXR?¦é¥ÿA?Øıi?«2,àÏ1X?´LìÁڌp?®²
­ã^§?ä	Τ­
?ÇðN$XØg?Ò±2		?ĝºÌ«P?¶Ì¼ƒ©m?¼'€ä­?ã#Dәš›?Îkìo ì?Ôn©«àn?ËÚ5|Iä?ÐîQ08è?³Ä_´f;®?á½Ô] 'Ï?¸…y_Q.?Ç,+*ô?®d«¼Œâ?º	å È?ŸG!Ge~¼?׾…B–ö?²÷'ö3ÅÍ?Þä/uʘ¦?´o¨½ÇxMIXED4FGL J2209.2+3710¿éu÷‹'EÀ.…yRژÀ:¸dàTÀ<D»ñ³6@êkñÕ¥@a
¿cí?Ƕ5?Ìt?Óóm_ÿÄò@õ*Ÿû ?ûãq#®°Ø?ïçz,ìÈ¿æàyó$÷¿ìܸÓÅ¿è]æe$G¿ïéºy
2¿èt¡B‡NUNASNone3FGL J2209.0+3652?îRƒR…]ø?¢øC¹©Š?•€Ãú?"RS? ÃHÈ#x?˜ÙìÖø?ë8Žù?À"†PÖK?¶‰ùƒ"l?¶ËÕ£1´?¯c<Àk—?°Àê¡úK?è׆¯=£?­tS{1Œ†?¯§=ˆV
C?ŸãÉ,sc?ĸ`®Z`?¨ñÚ¨vŽú?æ|ÿÖ œS?¡ßKKû"˜?ÄÚ\":?žR›n¶
 ?Á1äK?":`ç0?ì+ô°@¥?µSc~zei?±°oìç?®Ð5Qí?«
T!Kqq?¥÷µ´¦g?ä+Â_¥Eä?ˬOÁU¢?Ï~EˆÓ×?ȸßWªX?À@x;â™?º÷'Ý.]¥?å—<݀ú?±¯q轨ž?ºü¦.[?§Œ<¬â)^?Ì$Ķäê6?­ü¾Ð~?׀ éb7?«Ž¿KßñP?ג,4!¬?±‡&@Ú±T?Ðíj²â|?¨	Ž_ƒèMIXED4FGL J2210.2+5919¿ïü!
@
¶ÿÛíÒÀ9r)=æë\À;íÂÚ@l—ù±\Y@´¯Ÿ•\?Îpc?jy?Ï陌- @Ž_f—äŽ@·ètH&_¿ééÞöšüp?È#Á{4ÿ'¿å×<Èk.¿ëÚß_ ¡á¿äʝþ-B¿ïþé6ßUNASNone3FGL J2210.1+5925?å½ËM¼ª?Åvwý"ç?«ÈÓuˆ?¨#Âa
?ÑOha×û?ÄQJàÎâQ?Ù)宽dœ?ÆÄËæ6Äý?¼8f"îñ?¹w!w-Ù?ßÇò÷Ÿ§?ÄSÿž'À0?àzšò£å½?³R÷'Ç´Ï?»ÄŽBkÏ?¥ÎDéà?ئ–úzQ?±'Ê`¥¡?ÚHÊÔÏû€?¦Ïˆª8AH?¸tnaWj?˜«‡'³˜?ߚê%E?§ÖìòmV?àxfæéÙx?įâ8øM?ÀÎ܂³ŠB?¹}ke©¨?Ö§Ãð҇ï?ĖIx*D?ĪÓaÖ"¦?½Qšã_z?ɓÓŠ"¦?Å+f;¯iÌ?äpg²§î­?Åçwˆw³@?ÒʜúTÍë?¯ºÓ9cÔ?Æ@î'oXÓ?®ÆgYµ»Õ?á
uÞ9ÂÖ?³!ž5‹?Ân§IýÇc? «('ïç? dÚEÀ?«è¢jsr[?æ¼<÷'-?°$͇xRúMIXED4FGL J2210.2+1624?äî¾ßχÀ?€6†¤ÊOÀ:ë 8ÛêÀ<e¶ü@ôMãÕ@Ñ=?%¯½?ÍFž6€?"i:£ŒY?À+Ëö8+@0w±èDø?êð
¿0W¿ìÿÒ]°¿Þ^úâ3ç8¿ç›Þ¸‡›j¿Ú«žê;r¿ïý©^2»>UNASNone?ï°0ƒ|?tá¥Ì€À;?E1ܕ^é4?4ØîBՌX?' áåÍI«?tX°ab?ï¦b‡ß‡å?‡/_?àӅ?U³E`¶÷?\†Sf8?ƒ°õ_vàÃ?…¿¸•œÚ£?ï;tRbM}?ƒ·dUù?hþ"šš`?hÙK/Þ$ó?•qµ)6?Ðê-Mȍ?ï'þì÷Å?fVL9؜?O'A͙?4šì(ò?Nò‰þN®?eªÌÁìùX?ï]m ?'P³Qwu?Y2ʋ‰ z?N]ÏÔÝ?šŠ‡³4õ?ëv}'.:?ïP`ü«H?—~'¾Iul?cH™Bo³?q(P\Ã?›Ìïåß ?•—®Q;S?îdþQª¿?"˻Ā'Ð?vg~Lg?u"#%!Œ?¦ã7"^?'x†3M¦?î"Ú¤ô
%?"£¥©JÑ/?a…{<|×?R|.X¾Â"?¥™ýúc«C?"FNãyÌÊAGN4FGL J2211.9-2924?çb_VãÎÀK|]¥qÀ;X°ô)2À<Ìõ¢®ì@ºò°Œ$?û'SÚr§½?Öã܉Ù2?É_ÃõbÃ?ò¹K{(•J@{ëöD?ïÿ|'1ž?¤Gò\ÿ4~¿è?k*M±¿»	<¿¤¿ä<~`ƒ#¿ä§f pbêUNASNone?ïÄ°y§?±GdF?:÷øâ6ç?P7­íPnø?ŠúTÔÊpr?°û@–ü?ïښmÁF?o¡Æf'¼y?>·tŒ}ÞÑ?H¢CÀ5x?pÇz~Ôwã?k½AÿPÅý?ïxš	oÚ?ŽËá•f?n҂õtc?vdL€ð)?™Öœ€êü,?Œ'¶¾pþ?ï·åÞÛ[ö?^y$_?GðCkaÅ?22šQ
…m?€‡"!B?]HNϤ?ï¼·
rÚ=?'w¥3áû?@	>êöcõ?<Êx@!èç?£Qc×ä+?'ÜT‹:?ï˜ö1†F?ˆ#Åyˆ?Q`F†^?bŒºÌæÁI?‡Õöl-z¸?…'ìÅô=?îà)m.?–¿Š_™>?tȶ$°1¸?{;´:÷y&?¥Hé&?qê?•}‰ß
"·?ïRá.-ºÎ?xñA­"±V?RÕO ü¸A?I랗_«]?"v…Gœ©?x…'w‹MaAGN4FGL J2212.4+0708?îG»Æ??ÀC=lß&k¥À9ù틉5žÀ<'÷‹½8@A•Ò¯`@Äô@¯¹?¿: 8ˆ÷?àÔ=ÿêÜW@ñüLY@DeÀN9I¿é›¸øÚqÑ?Å¢7"/ü¿Þ€Ç%CŽ¿å˜Ôýó¶F¿îŠ4¡È<D¿ïóðÈT˜UNASNone3FGL J2212.5+0703?µ<,¶TV?³Ø Â?ìÆmàXDæ?¶b¸v/…t?'5SJµë?"keÖRð?ȕŸ¾:§‹?Ãye¾î	?æH^ÇWÿ?ÅxƒÿÿT4?¼'ÊJïðò?²¸/$Y?ܑŸ;Î?®÷+ÊM"?èê$4#?±¸5ÀWÿ?´ÇŒî{ÎL? bŽòIÿ–?ՐAc=£?«Œà?ô¡?ÞÐ
·¬1Õ?®#JûÚ_?Ç?b‹»_'?¤Õ"VÎD?*Ö\1s?ši›<@~ô?î¥F¡è?¢ Ã€CÇ?ŒjA û?‹u›>ˆœ‰?´Ÿ"ös;?´˜‰eJö?é§_4Ã×?Á'8L¼`?¾%ãe%ÚÁ?µÕý'Q‹`?¬4ØHݽ¬?ŸRc̙{[?ìxâX¾ø?¥Ù0k)Z?±IÌǁNî?œ|%Ù/;?¼OºVlb?ÞÕDîp?åAÔTð6"?²xÜ+?ÌÑ%ÏñF?°Fý
³ýPSR4FGL J2218.5+6822¿í‡¹›}Ü@#"Âß
A1À:ôنïrêÀ<Xu²3ÄS@ È®Õ@
â?þç,yێ1?ÏhMÇ3/Ø?Ï`•ÁóªÝ?û>[ØÉ@Tdù7¿æ9€ô¿ïÕ E…EO?ïÿat¿ãsBí»¿å{:3µ¿âÚ!I%ã¿UNASNone?î	Ö ;<?»YæžU?d¨œ
¹±?yp|–ˆÖ?­"Øݯѝ?ºG&/>±ì?ë§‹ÿ}#?¾˜i¥­pˆ?|Xi\?…N'Ë?À֎RÐ?½iâ>E'c?íhvk
·? —‰d'PÕ?r.¼ö|ÞÍ?oó³-›!?³œH~&ª? [ç8\2ž?íðÐK¡,û?d"\Ì?fßÒàx€c?XôˆžÐ?¯"þw´Ð?Œ±Ԙ{À?묆æ[
µ?¸Èqö^ãÞ?p|G*ä?i}1;†ÈÂ?Àͻ٤:v?¸Š¿+{8?çYÐóÅVƒ?É¿»Æƒ÷5?…}Nƒrp?"…%+íö?Рs¤"Ź?É¡¿ò•?êdjxCÞ|?©T.ž"q?€%|E³¯?xпG–~?Ål"ÇG§´?¨íIõ†™?êmŸþìa?©oê£ÁH‡?v£˜û«ÞÉ?t2-CÃðÎ?Ŕc=«Ëå?©,÷—Â"&AGN4FGL J2218.8+4736¿è¤–óՂÜÀ¬'ªÀ:ã5ï¦À<À®	"&¹@©¿©MÂ?ÿDâ–?Ë0‹£Œ·‰?ãæÀhæH@ªèžºjÊ?ÿ½Qӟ¿ëø˞#—	?ï͚R&=¿Óý‰ƒ!7¿âȅufοïUŠáoò?¦M®ß{ûúUNASNone?Қþ\D'?Àš_Ã?ášï/"Wn?ÂÃ(¹Bè?Ä`F¾E?´'œFà¾?Ц6Z¯ùØ?Å­¸›£›6?Ð÷'Ÿ­¸h?Àϧar$¤?Þb8¢MÀ?ÅD{"=Ë?Ùc¶¾Žy?´´‡\g'?ÛɈ¬ƒÎy?¶'ZîÖ?Å¥'›{F?ªÐGæÕ~Ð?æ{zƒÃˆD?¢îž'pÃ?Ê«'­
·? ÖÒl?¶Í"Ƨ-?'ï£ã…²?Çó]&Ä?¶Z݊ùÝk?â;z=o†?ÂæQ¤à}?Ïô#ª÷\e?¼ÑágA5]?Àßy[ÐO'?¾cï¯"?ÕZĂâ"*?Ɋªž#Áü?á¿gšª!?Ë|õ3ž=?ËTPY‰´?±ÁÓ#Ò8?ãADK'õ?ºx•Ë¶f?ǦžzT?°ÍEoÃ(×?ÜZ4vK®?¬éëŒB¨x?ØBªü廩?°'8X4j?ÇsõŸm²Ð?¤s¡^ö5MIXED4FGL J2219.4+3229?́—íá´À4F¸Ø#B$À;r:âTÀ<ªXÆj²ü@!i´6Rø?üÊáö)½i?ҚÂïH£?¿Šk©F_á?òs§Ös?@å"…à¿ïþtDuzÖ?ïõ´bÕ¤?Ý:ÌÏ€¿äTíB83ﻥ°Bi¾¿Ùœ	€²BUNASNone?ïàdŸšm2?^ÈÁ$ï?- JÀ' ?õ!‹[4y?mÉ[Âã-Ñ?]ý)Á"l#?ïÔìUuŸ·?t߁8±m½?Aë<Á™,Æ?P·æ*Õ¸L?sLm›SÍñ?r¦ml[õ'?ïSqÁ…¾=?u³ôË?[¿Jȗ[?Sö§Wðq`?"Õ×H·åñ?~Á!w»Ï­?ï"g³õ?nB}Lâª?Aj⣉—?2è'÷g'3?ÏeL"³?m¡!úÀ?ï¹Ývƒâ?sJIsh6Þ?Cxšé«'²?6,åݏ?€Q4þŸå±?r¶¡ÿ"L?ïÐH{*?hp¢l‹u?T—F"ç2?kÍI•f?‰øöàíL;?ŠÅÎmB°?îÌùc6cÈ?‹-#cWIZ?b«ë׫U?a6Äóöð?¢¸®`9Ì?ŠX»k}1?î¶ÚöÂO×?Œ‹f6~?KûX"L'?HŒÊ_—Ö?¤"c0•¸Ó?‹Íܕ]†AGN4FGL J2219.7-6837?Ô&)ØÀEqûçl‹DÀ:ãsê³g¡À=§"ïQ@¶`Ï£–É?øvd«{Cm?ʶI'¼1Ÿ?åU2âUu'@	­Ý|é?ûÚý‡TȄ?Öž 'ðÙ¿ÔÇå</[7¿´•M.±ï¿àµFÓù縿ëљ_â隿ïo)­¯PUNASNone3FGL J2220.6-6833?ã¹þãd,¿?Ħ§ø"5?ԛn‰(:å?Ãlçݧîú?¯""Æßß?£ýÚJ‰?à°ÞA"Iù?Ìç#æ<?Õw,œÁ`?ÈÍð"iü?ÂN-ÂRl×?·‡ۏñ?ÚVŸR¯ê?µŸùmrQà?Ýò̉8«÷?¶!2NJª?¾ÚP]¨?¦æþQÞ?èé›õ
ûÔ?¢¶u‡Œ?ÁËQj´\q? ÎIä…Ê?µ}'?h~?Ü!¸é>h?Üò'.@Z8?Âųñèß?ÝVȟҪ?ÂövÊjP?¸0\#5qù?¬éâUWó?×ÁAa…?͆š£Ú»"?Ûçݹe?ÎþÎÁ]qº?ÊÂgC0+?¿h…ù¡?ÑløKM(?´
%9¶µ'?ã¥Ìœ•?·|:j{?Àõ2Ü÷o?©ŸÎêmÎc?ãÖn¸´*Ù?±Ù@ØË#N?ËëˆNÇ?°ã-vm¶
?ŇY"à'?£H—攈³MIXED4FGL J2220.8+6319?ï´¨+‹Q¶@ßßã*dÀ9Қl'qÀ;%/<-®@` §@~Ú4"\?¿7¢®–*ú?Öík¾?j@»øáþ9?ÿS¢F'^ã?Ó¬îàóË>¿×>l'	Z¿èDîs¿é†ýY¿í'T~1‰:¿ïÿ΁ز´UNASNone3FGL J2221.7+6318?½KÆ'D?´it'¤!?æÜiZë¸?Ãƶ®ù—?Æ4¯p€?»Xjh?°p¦vÅÛÌ?±»Îr MÁ?ä¿9là?ÅEêÊ'š½?Ó°Wð›¢Í?ˀ\åG?Ïðdu'?°Çky	?ދ+º?´x9×b%?Ñói¢8­#?°á+ic?·_ôÝË?ße	?áÞú€?¦·rË-t?ÖkÈÕ5?í?¥=XêÁ™?²ô‡3·þº?©†ÏïeL?ç˜ÂÜ*…1?Âms«žSé?È"°óÂá?¾;a"C4ø?–—#Ëö³Ý?žûßþ»ƒæ?åħödÜà?ÉFвµt?Ó
=×7E"?È~4 ø?Á¯XÕ{"m?©4¶
j71?â;\òkº0?·JJé­W?Ò±™°jÁj?´Tò›t'?"$/wKlä?t㔷ú4?åKÀë?«ûú¶	ÔÐ?ԕ°üaºÛ?«6©¡ƒÛ³PSR4FGL J2222.1-3907¿àêJê	¶ÀLfѝìåqÀ;»HCe°^À='ÌÍ£Œ@ /ƒ)j²@
­¾Ìf?ϳŔÊ'?"½l˜À¼Ú?É B€-6ð?ó—8¦d®*¿îñù@É?騣ÂèG}¿ê^°Å/Iš¿Ð¨n^,†¿ÑÌ1|#çç¿ïýëóفUNASNone?îÏå¶Ü(=?ºçô…ùS¾?Pj8	?¸êê'é'ö?–[9j7‰ã?¦"+ÁÖ£?ïÄ9Nïëú?xlPÅD49?NÚ§­òé?Vµœj¡å?zÓÕ?t»·qµë°?îûÑËAåÜ?7"å×j?vÿƃaf?}ÞX¹ 7R?šÿã\/?Šž­ÒÙ?ï{<ëKq?q–ä å{?\K
"Rc?Hª®ãý"?·fò?ˆ?pì6‡Ä	¦?î߁Žcù?¬ž'?z•M&rß?§ÞÌÊ5¨4?‹¡î®-? £l÷½ ?ïaWHﻘ?'ÜtM|)?]˜ß¦F?lŸÐ°&6í?'û•Fª‡ž?Uþ`Ùä¬?îc®ìB?"¤TSVx¹?}¦_ùf;?'¥áPê_¤?¦Nç²™?'~X;#™B?ÐA?ŽÑj š°>?pi˸b£?eåâÍ¥?¥HoÅàŸh?ŽY	AKAGN4FGL J2222.9+1507¿ê±ê즦ÀA<fÙ×À;]`—Ì:À<¬ŠLõ|@éd'%ÜÞ?ÿ'ˆ˜ÀUÆ?ßuaù±?µVóרî?Úèpa'ëO?ÿßY´Ò/7¿ë°ýñ‡í¿å'¯Šœ¦"¿ç·ëÿ—û4¿Åóµ™ÕT¿å³ÿvmE¿Õ—®\õ#ƒUNASNone?ïã‡I¾n?]/›¸P""?0B€N¯£?$aYð7¼?jå4í†wq?[ܬK÷r?b9í?ƒM†Õ¡yŽ?VžëKË­?\Í<T^Aû?…ãiÌka?&©µ|–?ïs–þ½=k?~}8ǓH?\ÈÞV¾!ì?VC)å?$	lö?}AÍÛ5µ_?ïlèýk6k?py±ÄÚ¾?Ez˜!Gl?2è_C{Ì,?'·˜°'µ?pAw±IÞû?ïÉ()-º'?o¾ƒî=‰?8f9¶ñŽÕ?0ùúãoÎ?yå‡Ìòg?nc#.7?îïz®
ْ?¢pïX^¡?c¯&ú
ã?q[áÞ¹?Ÿ®4V)õu?¡Í¥›Í©Ö?ï j÷£C?†"!F'Û?e\a‰ÃœÒ?f…Å7;Zf?š fpÛ?"ÁÁ†.#?îOdyŅ?'¨=rè…?QoÌsèn?P{Œ¯ÐŽ‹?ª~:	',?'1¸Q5AGN4FGL J2223.0+2704?ÃEv™[ӈÀ9£œQÚ¾À;0<{±QFÀ<‰SŒo¬@=:ªËÆ?ü««u+%?àQ>¡{eQ?Û…;=ð?û»'øme@¦NTvÏÀ?ïñªÒ§a¿àç}mi¿à͒?2D÷¿Ýi'z™#R¿ïÿüoQÇs?îû¬ž¯7UNASNone?ïÌ÷Q۔ç?r«c"€v?PøËqÅ¢‡?Nb7{øÁÌ?uF$Dâkó?pÖÏ£¢w0?ï¡ÞŽ¸Œp?ƒ½Ó‡"o÷?`éÑN>Œæ?iFZ5`I?ƒMçñ–²Á?~Ý.+zïÃ?îáì56²]?'3Öró$–?ˆº¢Â{ÿÅ?†îäš`ùF?—e'ù£'l?‹%§,ÊÑ?ïe»=$Æ?p¢ãQÃöö?NŸo£Ô?<(º°ú[?Ž<š(úcù?pB/fÖ;÷?ï¡ •¦Ø?'D4"ÿ?d8cJJ¥?c3N¢o?'‰ÓH©÷g?Î
IÕ?ïl§?Ÿj	c[?rT¤È¥ä?†ÊÒ·øsR?š
è4­ä?˜ŠDŸ¾¸?îbßØ1É?˜†á¡";–?Žq'<ÓÅå?Š'y¬ÂªÛ?¢5ž/pÿô?"ããCû+?î¦VÎÃÇë?¢$añþ?Sí~'G?RŽÞæ?¤û'"4±ƒ?U"¾V—…AGN4FGL J2225.8-0804?¤âÕ¦ÀITÃóà7
À:Õô_¸Í<À<xÀ²¤-@ z@Ï~?ýæp­E£?ÈëæB"¥?À›Æ…
ƒ?ö×#gäè@ö/ýV'¿ïÿ¤Dî?ïËŽz\¿ÚÞ߉gó.¿Ý6çˆ9õſَÁ#vQÁ¿ãU§11Ñ3UNASNone?ïݔf?oÁR…ßٔ?3BD‰0¢:?$4sŔdÿ?p¨J¤?o'œë¬¸?ïÒ!3ñ

?sÓRđI?B½—0xåº?JåÏ#}`?t—³+a:×?pë+¯Ë¨?-æ1?m­dƒ?X-°Ž³ÿ?SUì&tú?‰Pþ¸K@?jö|öÚ4?ïN;J6Ž?mªÀ)›šÔ?^q±î"?BÔ*™´õl?"X_›#ºù?lí÷ÝLAç?ï½!Õ×|B?n*­V#ö?H'³†õ\?<qJ<caB?~m"Õ̬•?l«"†Mw?ïw³Ú?ŒŽ~°¸"?T²U¦pY¿?bv/5
…$?¥¯Û"M?Š® õ€
¬?ï6ñ"8º?€åÛ¿–qß?_sU™+ãó?Nl;¡ÐÅ?—*§9
"r?€,ú;H{?îF¬ò3[?‡·Ä­ Ê?n4…ç·¿?])Xv^5%?©³í"!ø|?‡eyêBL­AGN4FGL J2227.1+6455¿€ƒ†]€Òa@Õw–9'ÉÀ9ÔyìU(QÀ;FT$D'ç@ß}­Õx@	Zìeˆ?ã…Üî'ÿú?ՀW¾­Ð2@'}ke©¨@¥ºIg}¿ëÓ>€ï)?ïô ~$É
¿é'‡ÂÀð¿ì(ԟÿå(¿Ô$ÀS퓿磢AˆáUNASNone?æ›.(Ô¬â?ÅNˆ·|·?¦:ùéÊ?¥eTYÓM?ÐDpûÉB?ÄCÀ¿M]V?àdÑ^ú.?ÍáÆGç9#?¸ÊM¦?»óÉøÝ?Ù0WÈá'D?ÈHç&·œ0?â­Rèžÿ#?±|uhÚ+|?»Þ/h«ï?¥ÿÍF˜‹j?Ó­ºbçÖ¾?°KRšú?åCˆ2
‹—?³[HØdo?°‹itˆŸ? Ó¤>y'‡?ÑV?7®?²|ñ½þðå?àJÖ΋ò?Æ6œý¯Ì??ÃȤgÕ?½b²Ê£Ô?ÕÜæ`´1?Åù‰cý'?ÐÀh¹/"¡?ɍõÍՔ?ÉiJ‰{?Èn"ÿý?áEy&NQ?Éæ6Ñßls?Ø31¬[¤R?±Yž_?È-XÏ`62?±fBÏ?Û¶!ëô@•?²cÂ/˜|—?ԛ7兼~?½OAö^Zm?»* ̝
?º ÕDŒï4?âMó»N?ÂÒZë³í®MIXED4FGL J2229.2+6421c?¸"<»Üµ@v2~ØM4À9÷Å&p­À;k3—Ý÷@#Ü­ ¡@Ÿ!Í°"?Í,õ×]?¸'à™³Dæ?ñ`Ñ·Xâ@FŒªó´?ïÉ©—=žÇ¿æbڻοë$Äpù¿Ûg則¿ë¨ø5u¿Ý¨;¾/áUNASNone ?ç7e¯²4Æ?¾êŸÛۑ?z¼'¶4P³?u‹;Ÿ ¿?Ñ&BY–Ê1?¾¡oD*n?çk*ùM£?À­d¡.'J?"jꄘ«ˆ?•+‹§œY?ÏåúŸ‡´?¾Ó{°®Ó?è÷‹Y\_?®ÎkAXy?œœÙàž F?'ÒI—j½?Ȑ—b¡z?¬;Èö?ë3ˆià2I?•¹D>ODW?ŒOÔ]øŸ2?j>OǗœ}?ÁláWzæ?•D‹A´x?àãªe€?ÂÎlià™]?ŠKQeŒòx?'(¤¼Ó?ß+ßn‡iŽ?±_l×?މqjÐ?ÆZL3J? pÀn…ôÀ?¥H¡h÷¹€?ßhv‡¬îF?ÄûZ7ó¦?àÄ|5@æ?¶xk}zʺ?­¯.££Ö? :"Ž?ÚÁù3!u?µ'8À@?ãLµ;ûG£?©ˆÊãjRl?£"|{üzº?‹ÃøÒ_ÿ?Ööø‰áb?©–¶€Ô(MIXED4FGL J2233.3+6530c¿èš+ì(Bû@yw JÃÀ9¸3¡<]À;U¡ZX;*@¹–J@6>Ðö'9?Ä×ñXP?Òc^߉gó@Gª%Øם@ÒÒË>'¿ÕÖA?»VÙ¿áÞó?þѿ檀¥+ô¿ç9¾'‡.]¿ïÿþªJl¿ïÖ¯¤ÚUNASNone$?Ô(izþ¬?Àêk…×gR?ÂàÕdÃE‡?´:ôK˜?á3–>é?Â+·ãŽ?؋ª¸ÐÁy?ÃÏÃ`9?Ç 'Ž\œ?¸" ™S?Ûäð…?Á¡æhÃýŠ?ßÍåˆ|Þ?²KR@*É?¼öúrÍR?¢Ç¦hÒ)î?Øô[Ù¼ì§?±q*ÎÃn–?×*ŠìòJú?¤tbxQ=?ÁÛéhlƒ"?˜®Stx C?ßç€^×s;?¥‡£ÿ¢?Â/ÀF…V?±P%E—‹c?ȬïPŸ?¹>ð-̂T?ånä²¥6ä?¿ê ?ÄÑCÁ˜2´?ÀG!Á`?ÒO[m T?Ä.ñUÔY?á¤Yã)?Æ)e×Ê?Ó+¿¶ä®?°ÞtoŸ'Z?ÃFut5A?©ctGê><?ᘂljۥ?²õUh»uú?À¡ƒ:˜¾?šgzƒ@÷?ʘOUŽ?¨Nà?åPi"m?ªˆI4ÆMIXED4FGL J2234.2-4156¿àU¯Jþ"ÀM2ÃC·õÀ:¡HËJìÀ<ªº€™îS@etùÒ?þ&~3⅜?ÁÛY£ï?¿5£ÐÕ#?ý'ßäÅù@
šZ±ý=®?ïÄÞ˜¯¿ÙÖä¾0&ä¿ÝPd[õP¿Ý_Z©™Â¿ã7PcÅ¢6¿ä©N½þ'äUNASNone?ïùÚOÓc%?5®Yüj2?""æšS?…1'3Ì=?D¤/Ö^6ú?3«vš†{,?ï鰑i¸?fÙ+$Òån?0g:þº_?=Ûu3t±?dB‡í5?dRSF'xK?ïŠÙã5Å?nÀí­¯['?Q½/ªvco?YÜòµ?zKGEs°‡?k}¨\‹d?ïÑ«p~Æ?RfßxB&V?Aä¸ë
?$J$ôº?u	kGyvÆ?QàïûÅBž?ïõáO2:?B¤[õ=î?5ÿWÃ<w?*~ØGË{?P'ýAÿê´?>Å$Ý9~?ï¼Ö©*Â]?€û;T'?AÓdŽ1æV?R¶"‰‰àû?Z>ß쓬?º"Hk(?節,M³?p½ñƒ3¨X?Wå áh–?[¥ÉU,'ï?'Å¯ÍÃ?mwÔ
ò?ïâäÄÃÇ?q/ÓaLZP?TœÂÁw®?AVpU)'I?""DE?p¼e>Ò²mAGN4FGL J2234.8-2610¿¾eÙä"sÀMǝØ'tÀ;~õÒ-_À<óPúÄW@ '®K½@Jv¾£>^?ËJ´C¾ñ˜?'úu7˯}?ÇnÕö— ˜@.$kSŽ¿ÍïßáÒmv¿à1ǂàð¿Â°…ƒâù	¿â$`JmŒ¿ïþÛ"31?ïø'K‰ÁUNASNone?ïÕOÖg´?fç¹lb÷?Vzr(8É?Y}ÎÑ·?o¨"ëÏ×?`‰?Ý»6?ïÇÌUÈM?{Ǖ`"?N̎¡È³?V?'ÈÇà¤?x ‡ý>tz?wÝ®M#å?ï!)¦ª'?ŒU
A"Çc?z‰\¯^J	?~W–†Î?•8tQ?†Ïggàgs?契â
ô?gˆÞ8—–?D*ŽúŽí?1pÆzSŽõ?…šÞ"Õ¢z?gÀlÇGŠ?ï©]é|?y5Ô¢€_?kñ¨èD?iš8¤ÄÝ?}z}TS':?sÇàç§gº?ïl­Zõ"?!'¿x?W6YYhÌ$?eÇg[y?>	…LÌ?Œ>6ŽµÏ€?î¦cDÚ
ß?'ìG9Æy?öhŽI-?›ÂF®?¡›ÅÑyè?$[?pø?îÔ¼W´œÕ?‡ó՞v†?XÖpÍ"Ö?QÖk¦©ü?¡í†þýŕ?‡Çx7ÙAGN4FGL J2236.9+1839¿àµ²üAÀ@æ$Ý/ À;+k¾"üÀ<²³	­'ì@ ¦·ÙÁf?ú»iGÂ6q?ÛGaS.Ô?Շ­¾êŒ?÷æê…Dwÿ@'Q8×·â¿ìÛ;$™<}¿ÔW­Ñ_ſ堕 ãû=¿Ö3ÍA¼¸Ø¿ÝÜæ ]ƒ¿ï÷mõ¦àªUNASNone?ïÓ8g->Z?÷Ãü?N¯à¨?€yª™!ËÁ?rÐLY?aév'9"ð?ï{²µÁºÂ?TŽ
#ø?c"Ж4Ò?m¦î±Aµ?Œ.lÞá?ˆ'ª‡´‡	?ïI#ÊVó#?†qá|ƒÊ€?o|íÁ'úm?qåuU» 	?'ëèõ6T?"ÀÇØ\¨?îšõŸSí¾?¦ÅT ©?^øI•?Jl¢œßp6?¥`1Šdèû?aD²Z?ï¨fó"? "èt^{Õ?eGßðo"? 
pa):?€""p5qÐ?ri8Öpnj?î‰}1Ä?¨6r#/(?s±T1M?ƒòÊD´]?¤ùͬˆÄ?¥úȘ«¿?îó4Ì÷{?÷«@⨔?n0óWÅù?oΕ>^0?ËSEºXÞ?Ž7XÈ0?ìç8fr?ŸS+"(Û?hytTÍw?c¼¾Nê$Ë?¾Œúœ5Lµ?ŸA:{ߛóAGN4FGL J2237.2-6726?ïÜXãhgÀFq€AÀ;¼Ì¤‰À<Ó+—]7@ 3M«?ÿŸMR™*?ÏäÄeJ2?¹ü*9?Á")Ǥš@÷Ÿúêü?å).—ÂÿÄ¿âæŽà3·¿âoÒá8ꂿÜ)•»»¿Ú½ÒÉfÿ¿êKWÇýUNASNone?ïàÕ²{?¦ØO"–98?"f-Yܧ1?¿/VóÉd?nêÙÇÃä?¦Ù!Is3?ïÞjlìx ?lu	¥ÆÓ?4ãè@½?A¯TNù¶?nù2†¼ÿo?ij'»Dd?ï‰ØÖñ=ð?|òmÙ¥É?S0º
 —?X¡Ó
¥µ?‹#Éèÿ£Þ?|$5Á.?ïàdü?O:.‰D?2¨Rhïõ"?OŠ_G?mFð›†HL?NúåF
Óð?ïß^–¨p?m£¸Ã¶¼«?3'oŠ'|?+){€R@'?n?÷#ÓèÍ?l†‹nas??‡®,?…¿-ðÃ?D7ô‰ÕÊ?S©—áÜ?‡'˜^ey?"¿ì›øƒ?ï"اÌbD?ˆŽJ1Ã?Y°t½Ç?R?YšÉjý°?š	ã·'§—?ˆ…ž?9´?降­N"r?kŽos±?B¨»	|ò?4"ÿt&?"³BpöŠ?kÆS͎¾÷AGN4FGL J2237.6-5126?ìtMÀ
ˆÀK"DAxpTÀ:ÏfhæÀ<bÜ¢c@kíR@…c¯˜?Ó4Ú–Ž¢?ÙPê°£?ø
e~ßÙð@äÀ»!ª?íÁI̽¿èC}ÎaøC¿ï#¤FÞâ¿àhŸ[zz¿äk¼|±¿ï³¹€iÇÅUNASNone?ïáZ	O£Æ?s¢±b9ŽH?TV]'|?W½þ€á€P?dzïn' Ö?oþƒÂÜwÔ?jHÚ?ŒyÀÞ?hö¨è'ã?{&·Æ˖ð?6¡'x¦?ò#Kœ$%?î!·‡ŸÞ?žc¿n´K?‡ÂK
œ˜?ŠŒIíqù?§óôÀ?›#>"±;]?ïÒÙ
¶[?XކÞ)	D?W'½ÁîZ?CZÝ~  J?p¯s4*Ù?U	܇pÈ?ïÌ[`‡?|g¨…»@?j ƒ"~êš?pD'3?iP!6£®…?q2Ý«È?ïÏ%QÝ?£QªJI'Þ?{J£WŽ?".Ð4?–sr~Ò·Ö?™]•È®Îî?í‡4kÿ?¡\,Ç#?‡Ã}vUû?Š0¡rù>?°ÓwÈË?ŸÂ»ÓŠ"	?ïV8æŸË?&º$æ¬?ymZàñÿ?p&F$ÏZ­?îÂè]Ò?zä¼YAGN4FGL J2240.3-5241¿Æb5m9ÀK[I@»±òÀ9Ç]b±¦À;',kûÒ@ Ã-nÎõ@4M:'£?³ÈJ±ÿì࿦nJáO»ª?õöÁ]-Á@eÎà"j
?áh æ)•%¿ëšJ~©SK?›"*zä¿åYa/ÅÀi¿àÖÔBaúF¿à¡ýì)‰fUNASNone?îë§Ko?—ð×ßsš6?O.zŠ5Î?RóW¬‹x? Ñ"燭?—¿—¼<?ﰉªäÅ?‡ȎšO1?Y²©³‰¯?i¢QTUŸž?€§@ÿÖ¹?'[á@¹æç?쵬O(Ý?¥!`jøs?ymï¤?žQ?€¦®žš$¦?¸»¾ŒI"S?¤¼,]Úeb?ë9{Ä?—¢—ɪ?k§ÃŠ<Ý?U0§"¨P^?à {Æ!ý?—–}i`?í^ø_'yÔ?«•Îp×Q¸?i óßñü·?f+³Ýɑ‡?´;5bYÞ»?«#3ÇéÊE?ïJÌ@y±Œ?˜l¾êíç?d®ßŠ_Í?tÍ2GÛ?"›ú4›?•
Ôm¡?é0A‹þb?²¦FÁ¤?†èûÎåMD?†F"AðD´?ÉÐkÛÎÐç?²uW½z?ä$¤ú;?¬·Üu˜OÆ?€ôkv—s;?tPäEMµÀ?×/ˆìa?¬àôØÄÞAGN4FGL J2241.2+4303?¹&ú¬{À+dî
öÀ;µ^>JÀ<Ô6>@lf EoÌ@øBf¬ÝC?Õ5¯D%ɾ?ïÿÜ>Y×ã@R%1ðÃ?æ -Š&ßé¿êŒëÖ}O·?k`ñ²_¿áæ͓œ*¿ït¸¤ Ü¿ïñÓíR~R?á 1ί%UNASNone?窬ºÄÈ®?ÐMtÞµh¾?ÁyÑ#÷B?Ç]	pl#À?¿¶÷ãÑÌ?à 
ÏBë?ÐÀ6j¹öö?ϓW9'Šñ?ä"<¢óŠ|?ÐDZb–¬?¸ÝA@ëlE?µÒ¦|<LÉ?ߑéþG)p?´'½§Cdÿ?Ín…ÞjÇ?°	Æík§?ѶÓƒ‡¬?²£óHcPo?¾cûÊ^?¢Zr )Ö?êBÎeܱ?¨kalÚì?¯Þ.Oë3?–nNZñ=?âȕ~"+?Òô>¶tÚ?Éòä/-Ú?Ëió00@Ý?Êë¥!"|?ɬ²÷ŸÅi?Á¼î'»Zß?Ér\ÃT_?çÿø@C"?ÏÓj[úŽ?¼†a®pÁ3?¾þ$PÊÑS?Ö}p´yß?´Û¶bÿ³è?Ò¥G͟½?³{%{%?ÖÝH1¿b#?·Oºs‰«? '–\xPõ?Œþ"}Ív›?ìzМ¡G?©Ä1m—Ok?´¯ëoÄ?¥CÌç‰öMIXED4FGL J2241.4-8327?æÀôž;ُÀ@J^	}À:°Ù(û¡ÌÀ<…Ål†;@ýTÔî"?ÿ‡7|n¨?Êd_:£?ÛÍó}抹@Ê%ïúÏ@n½:2«Ï¿ëY@¹À¿Åù'¾8ß¿ÝÔ>{eÑì¿Þ²	Ò癿îåvå¿ï裝SqUNASNone3FGL J2237.5-8326?ë'ymC??µMí™g?µ²1ŒG]?¯N^zè15?±ò7­?£OYyUòÊ?î#ã±.¥t?©€`û"¥?—ঋ? ï¬È5é?¡ÑqªÅÄx?š"¢ð
!Y?ê;ª€qªg?¯€[¯u?½—ïW]¬P?¨ÿûeë?°Š¼¥'óõ?œØBvÈm?í¢O7ö'l?ˆ÷TçŒ6r?šúÙà€Ú?z‡^e´bd?¨]Ÿø–DÊ?ƒ3˜ýøæ?èiMc"¬?»-V1\eÔ?À"Hš!‡?´/jJÓa1?»«¯"?«ÿQóöÓ?ê#Oª&?Á± ¡º7?²óðrn\?º‰ÄíãÑ?¹õŠM?°ÑŒ­«|ú?æ.¦Ý«Ú?·Qt?ÉڌU/Ô¦?³h
Š¡?ºÕ°m'÷á?¤ÐØ9ÜRx?겯•.{?¢€‡©¯?¯OÎl_?•×1>aE²?¿ºÞÁI"|?=ÔÊPKAGN4FGL J2245.8-4148¿ïù⡗·9ÀN=þ!ÙnœÀ;"E	Œ³À<ïð‹î¶,@"Y‡°¸ð?þ'Ù--_µ?ÓJ"ä(3%?Ï8ùÜ$ƒ˜?÷çESÇ'q@_Î$1?Ò¬cû¿äì¶wò¿¾'¡T£ñ¿å}Ä@âl¿á°'¿ŠÄë¿ïøž;ê½UNASNone?íD"Ðp?Êé¯Dm¦?eþé'ށ?'ž£"{>é?³UäŽwŒ?Êvx½ë?š¦g'?†_"*ÃÔ?a»p?–`…?i<+!'\?'æ}VN·?«#íõ™?î"T{,q"?™×0f¹?|°xŸhÀ?Ã…D²Àg?¤$©JÅ(Ç?˜…Òœ­f?îÔßzúG.?~]&U¤?eŸ=-ï?OVÝX"Ã?¡X'ݯ7?}ªœ÷̯?îj#
'K0?»,dÕöÞ?uÆÃ?Z?¡8ì¼¥d?¦½v}Ë?¹ßÊ,=Þ?ï!br³H9?œTlá!:?n«¡Á±?|%ÿƯ´\?—þM؍æ¬?˜¢Òù˧?îמbP?›ÆV!Zÿ¼?'þ!ÍNÔ?ƒšØ=®3G?ª2ýÙ49C?™ÁLî0¥?ì¢Ãt‰À?›¯ 
ŸL?s3g‰žq?fµAÀ·E?¹¶³<Ð7]?›%1–9¹AGN4FGL J2247.7-5857?±G™­Ì¾ÀIÔÖõD»À:Ñ×ÙôÓÀ<&0ì1@£Ð3ç¹@¶½2%?½5 á6'7¿¯©¬â Æõ?ñ7jК¸@"'[d±?ïüL·h·y¿èMW¡§…¿éHÆÆ"¿àMÉåX4¿éóaáòN¿ïÿ-½R†`UNASNone?îø^ØAcç?µRƱ¶¹?šÓ`ƒ±!Œ?µgüvÈ.9?xƒË
&3?u1`*þ'ƒ?ï¶åeþj?z¸à¢êÁ?S»±Uÿº+?XßÈÅôD?€tá68?vL•î}"?ïOKÕôò8?"vlE\`?k«dhþzÔ?pç~Bñ?'¡¸	{'?ïùK2Ó?¦j?d c±+
?bŽÃló¾"?FgK4"É?ƒòÎÙâH?bÇVÍ3}p?ï^çö#?ª3q¸Ó;i?'vÈTH–?©áñ¯×µ?Œúµ™?…îUµH‰¢?ï?kÄãä?•UðŠ\³â?`í®&íø:?hª†œ~à¸?•ôѧË`?"ߏܧA?îÄSpYH5?ÝÃîk}Þ?wY6ÜAÖ*?uË5Àý›Ø? Ï¢g2ñ?Œv"䆜?î»kQôó?ƒæjؐû:?€è'(¥ÉO?l[E"å}? *"&Úy?'c'v캹AGN4FGL J2249.4+6222¿émœ µÎ@C±Ã\
ÃÀ9±úã`	À;ü}"€U@;ڌ(õ@¬{­?ÓÈD½IL$?ÇÉD6¶Ë?þzŽÜ§5d?á>ÚJ± –?ï­Ê¾­	¿Ü3Յ2à¿ëÝü›Çq¿æT7ûr¿ì©c`Íu>¿ïöQ*"ÿUNASNone?áWƒ!{j?Ì'‰|bt?¼Ö<2òVÛ?ºMŸÎšŠä?Öjãsv?Ê^3D®ŽQ?Ô$ýø‹8û?˨Õg·/"?ÄçV­?À¼ì3^@?à³¼î2x"?È|µÏ@?ߒvLí?²¾€l—šö?¼V]&C-?¥wj¬K?Ùkt²hH?±Ž-Ycé?ºXBWy ?"ö¢¹Fì?͈_â‹v?§z9ƹý?åRäßI¯?¨E)»f¼?ÛLJG6¼?ÊRFɽù ?ÊÛ<î9'?ŊÝϏ±?×F@äKÄ?Ékuˆ²?¼GzÆxR€?Àö2«½¢?Îv¡"\:`?ÉdO QC¿?äÙhBç?Ê$½‰^?Ô2¸u8"?°§Ãy5!Õ?Å]ºùÄ/M?®¼µs,?à÷åTX?³iúôÂ#?žzòu¹ý?'ëµ?ÇQ?Íåo¿ð4J?³Þxµû"k?ç–8pE?³¤_óÀ–MIXED4FGL J2250.5+3305?ʬ¬h~DÀ7H`RP/À:<GËp¬;À<cþcGÍõ@cá4¸ÄW@ϑE7A¶?ÂBˁž%E?ãóÞ>d>Ä@f<ù…'@çâû{9?ÙZ…<ji€¿'Š;¾Ù*d¿âÖV¹J9¿ë²'LÃýñ¿ïÿd™ÝŒ8¿ÞBÛ\\¢BUNASNone3FGL J2250.6+3308?ËÛÀStÇ?ÁWÿc€‹‰?ç¯h¸?Ä]øiRæ?°¯¡·®?­gtà%ð?Êà9YEŸ$?º»8‹ô?åÚA››?Äinƒ–M?»o,ëgäã?±i
*åû«?ÑO'øcöÂ?±ýþ2 f<?⋚¹]É?´z
Åò6@?Ã3Gž,ÙÛ?©Tu…åž?ØùQ"aS?¦¤DŠ¡î£?Ý{¹Ç³?¨*ìÁùxì?ÃéI7ßô?š†Ø—s^?ºzäÅ£?¯õô
ƒvB?êd®'F‰?¹ü&Ÿ¯Ú?²_§&X–?¬|åEÊÑ?¹Mƒ*<J¦?¸-i<&?éI3hôFu?Á²…Ãù¿t?¼háEš¶?´ÆĊºØ?ݓ¾'»?«<ÄàÒå¬?å­¯¦ e¦?´P­EÀ?Å«®[¿æ­?­Êš«X ?Âü"[«¼? —?A÷V?äqž2c2?°loMóû?Ë?a+‹k{?¨
Ó`çUÍPSR4FGL J2250.6+5809?èé/ÑKY¿ðûx–ê'°À:§¢>ƒÉNÀ<	ɓ\i@!'8úóPÅ?õM
À¿?ß}~á‡o?ÝÏ`cò@I][û©Y?óüûhÁŠy?íÝ®ˆ*Ü¿ïù¦êºô]?îVÃ[4=¿Ü«›úœê¿Û1s?'½¿ïã¡ìõ6UNASNone?æÅgcø‰?Ê¢òŽ0
?BJ݆É×?™++°e–?ÒêP'ñ®Ñ?Ê¡&­á±?ØS×d?Ïo¶¬?‹Î€^½®)?˜‰ á³
?ã‡ý€?Ï
úOÎ?é%8/±l?®îÁ™[éÝ?¢Èk1YòÃ?—]ø©€‰¬?ƹvÜà?«gn¢j»š?௱©¥^?µ#ÚG+/?Œ™ñå'e?}œ¯%'}—?Ý»Î_†œ?µv'%O>?à/Zñ"*À?Éd­Z&ù$?—iFoÄì«?œ~0Œ«C?Þ*µµñ—?ÉLm
kð¶?ɨ…3ŸÙi?Å{rFïR´?‰T•º"#O?–6ëv•?é0Œ\;·‰?Åj>ÉO¥ì?ã­ÜÙN)H?³N…>mÎæ?«"g–¹¬?‹Ã›ŠZm?ÕCbŒS?²A˜ï®+Õ?ւ§>fÔ?»šÙ¤e?€9ƒ†Ó[?'"&±=Ò?ä}Ès)uù?»QDX¬¿MIXED4FGL J2255.4-3252?íõ¹>X3ÀP"ÊÕ{ÈÀ:ÎCr‰ŠÀ<¤é½ž[ @ÙIŠ8@¡ƒræ§?ÐYkáÐj?ЂƒÓ^·E?þV'Tà@ÙE¡Iç*¿ãÅâB)ñ¿Î	{(ë1¿â­×>?׿æì¶!9¶…¿ê`üßåy¿ïÌvÀü‰ÿUNASNone?ï±%Z"°ˆ?sâ$óãe¸?Y†lÖÃ÷¶?LáÉ0¾M?€…Û¾+›!?qÅnX&}?ïÎ^6¹qô?vì"Ó,ðö?L.S$þÃK?UPº}÷s?uKDù¨ÿ?sƒ€yÌBŽ?ï,NԂ?ˆ]_µ$íÿ?wX1˜ñ*?vîŽæ1?"§.Ú=`¤?"">F¨)?ïœd˜Âs?bÒ\)[Ï?biHß
J?DÖHgOß·?"L‡"—×å?`?²±cÑ?ï0¾jÎì?â@Š0[m?l¹C8%Â?cÆ(-D«†?–Q
<L•
?‹b±›±x?ïhš!˜šÛ?"EØ0Á?bîÈN¨¤?rP,lhö?ŽâÉr×?ªm]mÇÃ?îx_íÑTF?"\òf'Æ?ˆ_´¸Œ?ƒnä;·¼É?¢b|˜=?¯¸Á‡\?ï'©áz?~™+[Š¬¢?p$vÍ~ÝÝ?^y¤ֈ?™­ªB?|ˆÇÃ1ÎAGN4FGL J2256.5+6212c¿ïÿ2|V@ "S.{>À9r« ªšÀ:íև`±ñ@R°ŽES@Äg£}?ÐD~Ÿ˜6B?Þ¸AíHm@[輜$?ñÌGVUÍ¿æmE}¸'ƒ¿«iü"0·ê¿æÔS©Ë@¿íüŠ_iòã¿é!	?nÕÌ?Åáœ}#Â'UNASNone2FGL J2257.5+6222c(?Á'¸{õ®?ĽS·Pþd?Ã1!J¨oË?ÊÃî
Ú?æÓ	W?Ðd'ìH?Ð&*	2?ÊÛÀ!n?É;ðy?Ãn"¨á,£?áž(õö€?Ê}ÔÓ<¹«?֐}|UU?³0Kû•²æ?۟x€Å7?­‡bßã?ß¡³?CH?³zÔµhF?¼}ß
ßN|?žC/!"0ú?Ƥ­£*«¿?¦Y0;ê¹?æǵÙkA?­Q1lj}(?¾Ç"NíE?ÀA"AÕ|8?¿Ï´™áN?Ãr‡1?èFÕ¬f.?ÉÖ˜ 95?¸È3Ç?¼ìàå]'?Ò#³kˆ‡?ÉõסÖõ?ãêÍl–‹?Ê}rœ¨?Ì,•Ð?®V
ȌÊt?ƅ¯¬ÖbM?°0{"
ê?ãZïŠ3m?´¬oY0F?;"?…fqˆŠPò?ÈüêèF?±«ÄOHê4?èÖí±Bi?²†Ðà«òOTHER4FGL J2303.9+5554?ÃðèC
­ÀàÒ=OèÀ:Åc®ünÀ<^UªV€@!¸_õ‰Ÿ?üŠ"C"?ÈÁêAÞG?Åq!Àŧ?ü£mWò/@]Ñ8Â>¿ïÿø]ˆò¿¼ÙÃUU?ïÿÎÿYg¿Í7IWâ¿þ¿éÈ}ýܺ+?ÂJÆüÔ'UNASNone3FGL J2303.7+5555?êæ;Xp¯k?Ä3CÍô¨?xÎöþè"~?skUú`–\?àšæ[û:?Ä,•ózi0?çhJˆ©æ?Áµ£Ç?u´$rA?|Û÷o?ÐÛWöGU»?Ák_/̇"?ì™'"[øW?¢'RDêlz?9®¹º?}[CÙ¯Åf?¹ü¦
>"?¡§yg£?ìÍbx½xh?"t˜)î@.?‡&"å™]›?vI 3<õ?¶°'Þªëˆ?'XÔìü¤?èÀ¤	€k?ÁÔ¢rõÛ?‰ëcÜ`x?r@Œ|˜‰?Ëd'$*+Î?Àé!pâ?Þ3‹×¨â§?ÈbôTXÐY?{F:ŠŠ?‰ŒßÞÃÕ?௭Ÿ,wû?È6â4"ª?é\ÎC‰0…?©ÓVð´?$Æ£™Ö?†OÁD"•µ?ȚzÑP?©3.4W?èÉ»²?ªÞÙ_o`½?–<'ƒM^?'3VB	˜?Ê'í¿?ª1쮋æuMIXED4FGL J2304.0+5406e?è²R=h|ÀXàkæÀ8›Òß5…À:äk篧"@#7›!Ùï?ü-SaÅ?µpb=·Æ€?Ï>;¤ò@"è‹+B?þ§mrU¿ïÿêњ'ç?ïÿ› 'V‡¿ÜÐæ7
¿ºWìPӿفà•V"¿»?#@÷ÁîUNASNone3FGL J2309.0+5428?ÑUƒ·i?ÄRv¼Ûú?­ÊÖɬ?°FÆq•£Ô?哧ф†Q?Åüä'Ãz?×æê'æ#?Ïm'uU9?ÁIþJb³?Ã{ŠÀÉð?ßt˧ƒ?̕ºOOQ*?Õõeܗ‰ä?µ•	sé~+?¸hnk	?¤³Nón®?áø?D—]?¶…ÇÐo·?Å%IùÑÆ9?¡Eªº@g«?¾†ù²?¢EN'{%?æåêolkÛ?©ß	0"?хü3AËÒ?Åp·8R=?²øM	¯<?¬æSd3¹É?äÝøDäzW?ÆüòF%u¨?Æû[=ñÛ®?ÉöØö?Í'ûú'>?Îbùtu¼?â÷*pä…?вøp¶?Ò/Ÿ¬ûm–?³é"u6=?¸Í?>wp?¦!wKø?ãΈA镗?µÀÀ[ò'z?­¿çB63Ø?"rû»›Î²?ïsÂç¾?°™6Ë?ÅB?é8$›Y¦ÿ?±˜h‰Ç¸"OTHER4FGL J2306.6+0940¿ïÌU&´0ÀF£sÀÁüÀ;)Î悀xÀ<†\<@øï@2gà9@‹ƒVa6?Ë'4!o¼P?¨U:Þ¼þ?Û%l 9±R?û:µÃ›Ë£?îêI¥Ò?ê©érõÁ¿égÃd™¿ãôJ?>YW¿ßJDÝ)¼<¿ïÿ!ž5_³UNASNone?ïV:\¥Ðè?\*õ¸X•?Pq4çcŠ?H'IbB?"1¡‡Z?ŒØS<È?ï…/kõ¾Ö?Š?Q#´<?dÝÍJË??kIQ"¹W	?‰|±Æ%±?……'ÕX¢ß?îüÎb»®?ü°
{?u|[ün;?võ×ՙñ?›"Ÿ$8'š?Š'††À™¦?îÑѤè?€P~§3¸Ð?x†ë&_&_?c
&ô²V@?Ÿ¤"ß}ÿ_?}RÁc¥%p?îÃf
¿À?˜V'åðV·?d1r «]?^
Á'Ãs›?¢‰œ>˜Î?—¦':vVE?îÐ̀"}[?¡eùŒ¦õ€?tžÉàXwÀ?UKñL? _N¹h×?›¿LÓå'?îj²'{F?"bñ
•j?€
BÇ u¡?}…LäÁ×m?¥RNB¸tA?'°cuöEO?ìÓ»N¨¸#?™C½Vþ'? &_<ü?~ŸÎa)j!?µ¾ À˜Æ?—#UŸ¸¥JAGN4FGL J2311.6-4427?ᆲª‡AlÀOǛÜiøÂÀ;@­
ê¤NÀ<¨¯3+¦@TjX¹T @9×wJº8?Ô.]¶i‰?¼¸—
ÉÅ?éŽ_tÝÛ@¶ø¥Ò?âØ"ð½¿é³hb?_¿år¡L$œ¿ÝTŸÿå(
¿åly¥ÞKz¿ðUNASNone?ïéšÝÞºW?ƒÃ;Q3U?,KŒù&¸?ŠÔjØ3©?d¤]^×.+?ƒ¾9[ J?ïÆ.@ÁLw?yÚ×þ·\?Py´fÄn%?Vw#±JŒ?xÊrŸÄ·?uò®\¨À?ïtö­hP?xÑô)ž?`¨ï€‰…Ù?]٘…šû™?ŽÎFk섚?w©ìñ°?ïzfM'Ù1?k6urb?VÔúõ}eÉ?;Æê2á¢þ?Ž‹Í<Ú?j±‰?þI|?ïÏUŽãï9?pxsˆP¯?9Ñ¡lÊÅ`?7•l³*ª?v¸q/š.?oåècîr?ïsãåË©ë?‡²ªo?].­ëͯ?hàS"zk?a0Ø¡'"?óÅX;	Ô?ïÜO8}?…Ý%"Ìñ¯?hv±^pœu?d©ÝGl!?›ÕŸëS†Ì?""RýÙ?"¸-?‰'¢zL?g
îÿŸVv?Y¨ˆäÜ^H?¦T¯W6–Â?‰Àž]VAGN4FGL J2312.4+8253?íÀv£S	p@4£ èBtÀ:œZxòZ%À<EÇwù5á@̎²µÊR@½aÀxi?Ð6>"þ?Ôq³/lÕ@ã
ù½Æ @77F¾*s?î8Çâ'@¸¿ãÚ¨ÝÚ;J¿êšÂ
¬¿íÚ)vñÎå¿ïÉ4â_Ü	¿é8âií¤UNASNone?îÉ\?útƒ?œ¹8<T?…ÛïË£·?'
ÙY½~ƒ?›æ€þ³¾?—ä	¶Ti?ì\ÂøY?¼x'GvÈE?¯öì)58?¶ž)6´p?«|å1\>?¨µ4{mð°?ìÛÍôȜð?¡ì,;+Öò?˜#ì %­?Š™ÌoYÕ	?³•2ŕ?Ÿˆ¸"mØ?씏"¨¶:?|ÐùÔb?«Äøf¤À?ˆ"áN"j?ªòÄ¡¬¤?']7õr{?íÅñw;y?¨§"0f8?'‰JÜ??ŒÂ¥ƒ<?ª\C5ªsì?¥IÅI9Ÿ?ç&¾} 3Ÿ?Æèk?ÄpâWðÏ-?Ã
$/ÿ;?½èGgIJ?³´ì"êè?ê~ÈÖÚ(?¬±¥1°Û?¦†©¤jO?–tÉç¦S"?Àc2<Ƹi?¨÷͒«¥?ç'×A+)¶?¦ʁUñr?¿Bsˇ[?£¶jN—,?Âiiê)?œ+(ZŽ­2AGN4FGL J2313.4+5947¿âù	1¾$O¿è«ûèCKÀ:&†ZøtÀ;;ÌÛ…¯@ ³˜zµ¨Ä@‰~Jˆº?ƣ歰¿£$"3ÿ
?ÞÑ0ÿÒ2½?úî5r} ë?ïô`Å<µ"¿Þ• c!ãU¿è_øù{¿ç\¦>m£ò¿Ó4˜Žß#¿ë
Οµ½gUNASNone?Êðv9 ?º pôðés?ZJd]¿?NÕ Ò³²?ém°‰ ?º·Kú2V?ȶåãQÒ
?ÇCë…RBv?ÿÔĺp?•G!³¡0&?éZG4O›|?ÇþÒóZ?à?^k¬]?³£ˆ³%-?"ƒˆ¹Œ#?‡¿¾Ïç'þ?Þ9Ž·=nu?³ªÙ©ØÐ?ÜíK¾«ˆ?¬˜þl–§?ƒ2˜0sra?n*¦("í?á<¿ólì?¬³Ä%#ôþ?¸Ó7ÂM¾?®ÿÖì3»?eNôÂM°?[.9Î~ºÝ?ìЇJSÓ?¯f"åÊ£?¾6R%Öm#?»õiÓG)#?ƒ'ºm™Gz?"'Ž˜½.R?ëë*јl&?¼@7æ8r?Оï'h?°ªï­ºr^?ž¤$tïå,?J‹>‰?æ»gV½ã?±)©Äá?Ç3òDo_x?©›vî6?Š/î[›F?€<£-Cët?éÊC¶k¿õ?ª;Ã8ºMIXED4FGL J2316.7-3144¿ÛîØ{è¿ÙÀQ;27Š°ÉÀ;=•ôÉkÀ<Â"<jêZ@èák•O]@9þ¡[.û?Æ%]‡š"•¿±=èîÁi?è¹EÁ€=}?úˆÂ>SwÌ¿ãýž%ðU¿ì´R¿Ýñ¥U¿ßgk1|¿çŠ¢OοÕð?ÃdnUNASNone?ïÉ&Uf{?wÈ·†ïéÌ?>Ȩ £Ý?3-{³éO?y€J­>7V?wFTbÙÅ(?ï¾É&­œ?~ª}:¿ù¾?TŸ&犝?\0›8R?{ÈQ¿ò"?ys/›MÌ°?ïDê'ŒÈ?†Ã"îa?jåÙ#Ïh?rjŽXÉ|?"áß½ò?"9GÃdÎt?U='?k(é¾?WÌ¡[•_?Be9G)?‹E
ó^v?jðËgš?ïHKؽé'?–ßà#6~?Sêü"<û?L•«|þX?•·ÜŘh?•¾×Z‰'J?ï\©×²ât?"æzR>¿?cWùèZ8?r×
5c¾?'ÿá6B?'[ǯŠ$d?î҉i¦%?Žä¨í'ÁÉ?rú*J ˀ?w û1<úŽ? x$(#@¿?Œ›ËGó{ç?îzN|S§a?‡¥Á¿)U?qOxÃ,[?cªÉļ?¦1)"üç?Œ °z§AGN4FGL J2316.8-2518?ßwH"ÕÀQ/Ë>WS¤À;j@ºˆÀ<È)ösD@8bè,¤¤@7^nÔÊ@»·Þþþx?·Ç¡á^T@r»3rH¿ïûƒ¶?ߙС½6¿Ýåâþ"P¿åÏ\>oQr¿ïþ9 ²ýï?ïøª O€ÇUNASNone?ï=!ҞÚ?­rÁ÷Œ#?£Ôíù"?­+$LÇv?~ßÂø×zw?€°1û–?ïÒÁß;—ä?Ã{©'_¼?Måì˜,?gUú \´?râR…ü"?zi¨˜?íºW™'Xz?¡=^BY?'Aî¸»æ?'äšÈ
l?«9·mÖLq?ž"KÛsú;?ïæìT–I?l³ßPíG?'õÑä–Ê?1C hEŽ‡?h¹ŸbJ;Ò?lU@À¹¿ç?ï>äþዺ?¤×ÇÈC4º?ŒZ=?¤Eé8Õ?ƒì¬'D^?'	£+{?ï‹Ô"%ó@?˜K
2ÚÌ?^eÂFW?"Ö´2É??‰INsB§K?"^,"v68?íͲ‡@‡?ÀAÈ#$?ˆÚæ< ÊY?ˆQüdýÌ?¬îúBÏÿ?™¨è""v?ïp»ŒçG?«Ñjy¯?3(œs«?m\)8jû?'›îMŸ?«¯â]èƒAGN4FGL J2317.7+2839?Ð1…Üß{À=ÜÏ|ªuŠÀ:j‰á•²À<hÇåÝ?@ [¡äì©6@'U»Gi?¹nlŒñ¿—E`dø0?àšf³"?ã@
Rí*eYK¿Õ·¼]éÀ¿ßôYĚ̿âa8ÿûοá+8'ŽºC¿ÞÇ¢@‡.³¿Ó\åGB	UNASNone?ïøx7QÙo?8›îRQÜ? /æiw ?mþ»"5?J_Oòì"?6&'Ö
›4?ïâÜHV?i>püˆüd?1"ì{Œë?=áè7Ž'?kÈàh9í
?g'…Ñèì?ïȶÿ—?bæ\­å\å?JFþ¤-7?F%>ÁBhM?x[ß6Í?»?agVTæ?ïÄä.ù?ZêHؾÍ?;hš.Œ»b?qË6"'k?{×_]­¬?Z3Qt:‡4?ïòC¡6éC?Hèë—j("?16¨Pö!? «"ƝL­?W8°'Ré?FK‹žªês?ïŸbi_GÂ?†¢Ž•˜—?AƎ2aXN?QACÛ6Èð?‡
üÁÕx?…ÉÞ1|Ž?ï¢G¶€¸?rpw›ÉÈ×?Rí-ó1Ö1?T.Ù[¢Ob?…lšï]?qO*Ή ?ïH@ÉHÞÁ?y…m*æ^Ÿ?TC£"?C	ÐBǐ3?•³¬©ç{—?yėÅ<3ZAGN4FGL J2317.8+6140c?à›ø£.1°?é˜c8´|tÀ:݉³r‰À;"•µŠé@"»ï¯Ð¾@Gz>Š?ÉÍ$`‡;?׺šÛŽ½@
À?`h?ôΨB¿ê½˜]ƒ¿±dS爺ϿÚÈ2¾ïŸ¿éÖð¸»¿é€Å§J¿ïÿþÐñUNASNone!?Èý@#ì'?ºÉ¿ð#Â?¨È_ß÷gy?¤y·,ÅM?è4)øÌÚå?½ÃÆÿ-r)?¾Xº™Ìù?º²ó%Î?¹¦Uîã¼Â?±;(&{?é2
ÐNÉ?¾p[a…?×͌ ›g?±BoÜÉÔ|?¸ÉË͉»I? ]ò¼…å?áW_ÀY÷Ã?±¬ìb¸]´?Òý0@÷? ChÄç0?˜Z~¦¤?¢ßPÚs?ß4¢>XÖ0?¤iÓáǎR?²ús)R?¨â·÷{í¤?±+ñ]ÙW¨?±úRfá'Ñ?ë{3s['ª?·ÙÚ9X"?¨Êã?¨fPmµù?¼Æ~BêÐ?¸£í®ºU?êæã—r*?»VsîÓ÷}?ǹmÊ]Ý?ªÿÓ]«Cõ?¾Ÿ²!û¨W?§b™)­h?æk[`Mó~?±>›º¦Ç?¼%v˜HòÉ?•Î<h¯ú?Ñ"
°¡â­?®Â®ì¶"ò?ãêKÔ¥ðP?®ÑôÁíÒOTHER4FGL J2318.6-3827?Éh¨Ü"ÐhÀPâpdìé£À;٘áõ²À=Jb¹3@û‹¨jAè?ÿ@[ŠjQ­?Ø9Å^?ì¢E¥%¾Ö@šð{þ~ @Ñʽf'¿ïÿå=†ô&¿ÁPɆœ;à?ïú՞­«¿Þ$#á0±ú¿ìgs¬ ›¿ïý_ÂvíUNASNone3FGL J2318.6-3829?í¯dœŒ¾?²Ð­£ñõ?"y,âm:D?›¥Ö7…
?ªÍÉmš?®úAÒ?î"à°ë€þ?®²ró+u?'h¢Õ?£ra[åƒþ?›~ՀÍ\?¢2E¬Åa?ëš~[z¥
?ªÕµZ"•?¢ëÃk0?˜+ÖtJ¾?¹¶Œ•5m?§™³IUû?îm '¹h¨?n¾8ZEŽ?•pݘ	E?"õõ­D?œÛmZ=½?‡kûFtèç?ìż •ó?µ1t0c¹?¢½UÀ¹µ?£BzyÈâÀ?°ÔÛo?Œ?°›dßx'?ì·~a`?ÀûäVEß?¤Lº3f5ž?´^¶Á¡	J?°²
Eó0?µ]`ç{™?éâŽgâ<v?°üãÛ{+?§ñïý¬?›­¦\n‹?ÂyJ÷»þ?¯ôä$œ?ëÕO'@b?¬C·	ÍüP?¨6'jŽOu? â֊¡ë3?µ<aÌ	¶?¥Âà"µ¤¢AGN4FGL J2318.9+4151¿ÉbᒒÐcÀ1ŃùdoÀ;¿¦sœ°À<Ví½\ì@Ô¥Èüލ@™#²?ɖ÷¨Ãƒ"?®%{·?åcä
Öó—?þàUÓq+¼¿ïƒ"4?ïÅ(ÉL匿é$É®4[Q¿á@$³=¯Ž¿ëù—eâ²è?±qj{sé²UNASNone?ïSë4@úF?‡LӖ‹4a?eîc¥o?[á‡vÊ?'ÞÛ®l-ˆ?†œõø?ï!XÀ5?"FbŒ%‹?auôus¤±?gdðöñ?"Z,£wjý?Pc˜G^_?î¿WN¤Œ?"|T|h0?zµlã÷ïb?|>à? ³Ý}8Ð?'™"Oӈñ?îÑwC)?z\*I9æ?~·B6ZSä?aÌ£ÿ?ž/'"Îó?wPL‡6Òd?î·ÿõ‡ð¿?•')6$í/?u˜4î¶?oßZÒu?¡Ìú
›Úÿ?"ó0Ðù?îãøDõ¨c?žÜžè=4¢?yD|ßèÞ?`#‰Ðk?/Ødúc[?™ѓ·Ö'?î9Œúµú?›ºõ¿u{?€Â}÷#Mè?âE‹
?ªÛǵu\?™´Ã?지¦>Ô¸?–ýh@É-b?"s÷-$y¨?€=õQ"ú?µ¦ýRHU?"ªN;°ûAGN4FGL J2320.1-2440¿ï똛S_ÀQV灃ùÀ;75c'À<°Ô8í‡@"·ç7‡@'`}Y"?Áƒúuý]8¿µ)žŸgäÁ?óÁC|V'´@mÀÐj;2?æêŒÑ4;¿èÏ_žÌ'¿æ·Î8Ø¿åù˜¨)?µáVáRÈ¿ïÿÈb±UNASNone?ï'»Æȯd?¶Ë‡ã,ÃT?a–K;ˆ¸?{ð9É-e©?˜Õ½Áa?¶"_^žì¡?カ-ñLU?'Rõ!S?VôqÅ(?bEÍS¦ò?{£b½.à?}ÍÆbs"W?î¥n®«Æå?–phm³©ê?dii9Ð<`?eû´Nû2Š?¤b~~¤ål?–ì‡?^l?ï­êǽ!?jN3eòF?4£L((9n?(Á÷I‹®Ü?ƒà3¥×'?j…>yÖ?î2Š~ž–"?²Ïg3èP;?yb;ŒÂ?'ª'}NÜp?©«³ƒ/?±»ƒDà³?ïv»¥æ?"–Åq™?]
A‡óD?pù¡Ÿ«	6?Ž×héÚl?'c3	J_?횱¨óÃu? }AǑÊ?q‡IåñÙ?qPhtï¡?²þ	? 2Xá¦JB?î°~¯LM$?Ã*~Ý?U_¬¹ã
Y?RùÅs?¤M¥'ç?Åy?ˆ¶ZAGN4FGL J2320.2+0707?ÜæîlÀH _ZÙjjÀ;=®¸å;À<‰é'9Y@!
/ÿL%ó?ü¸âe+Ô?ÓÔR?´J*ñpE7?ãà÷?ò=æ*þ¿ìjœ&@‡?ïw·ÒiÅ¿Û~ž¡@W¿à؆¿L[£¿ÃÏ¥ïa¿ä­rÊ!÷¢UNASNone?ïPœï©4†?²×¼ÿã2?"±¦t¬ ñ?²É&œÜK?‡'—!'?ˆý¬ØT"?ï¥Ýô5Ž?ƒ$ódô?ZV‹û	Å?c ̒6F?ƒ=°Òª¹%?€j=(/?ï9ñZö›¨?"3$ýˆÔí?mƒXõ­?u8–RÁ?•i¡é¦ ?zå©	H?î‡!¶¢Ù?ˆ~f³m,?l$d{d+L?Y^Ìñ?­ÅG›•µC?ˆU'SÜë?ï=ݳF`Y?¥ðfͲ@?nŒ({Iüf?¥) 
¼w?"rÄ~Û¹`?ŒTÞ¤q¬?ï0ôs|?›Ei·@Øê?i——Ä&êá?v[s9¤¹£?š§ªÐ|?˜í3Œ«g?î¢ëÛcq?'­'iF,Å?róJl*v?yoö"ª¦'?£rØùKó?"­/…Y?ëFèÉÏä§?¢öûˆß?uG!ǎì
?pj³[Ó	?Â:#Ê,?¢×íAGN4FGL J2321.9-4842¿ìvˆ&CzmÀO+Ê! áøÀ;'^±ŽÀ<™Dwÿ@ð³¿Õ˜?ÿÁ†}]"ñ?Ð
,8m.Ø?ºxîÍ?é¬ÖÝÇÆÔ@?X£Q?҇±d¼m.¿äÛ£ß¿ßfÙRí¿àìÒü'¶v¿â-«¿‹ñ¿íù> #ÌcUNASNone?ïã9e§N¹?VbÛ!ñ?4¢Ç±Ø¢?*´Àb7?j2A'dО?UH×á"?ïÆÝAd?z+ê'ò?N"êcP÷}?T(Q	°Ê?y,V¨^Ս?v"‡|,Á•?ïŽÄ~þx?k
½tÁ{<?Z'¯ø?Sʛ^[¦'?‰{eoÿ?h¦ÔTPp?ï:$sIE;?sÏ¥tÊ?UG*^"à?:š	*r»?—fþñõì¥?s¦*º©_»?ïÂ/؛ô?jkÔ&?Õ7?Eö€‰*??<|#/†ØÓ?|5—ôÎRš?hÚ×Ct§"?ïuptÝ!¯?oŸ¶§?Y«ŠT¦¤?fH'''R¡?kRõˆ?Ž6¨(j¼¾?ï;#ρÍ?}ÐÕ×±A?ce.Íܸñ?V¸cê¨?–2u­ˆI?{xèABûˆ?í»ëéü:?'G¼M‡ó?fZ©zÕa°?Vú-\÷S;?±mËdHÓ#?'i]®à<fAGN4FGL J2323.1+2040¿æ™»}oÀBÑ|o½'=À:ÚýPùØÀ<kymª'†@¯ˆc'Iê@¥ÆÁ#?ÃõB6Ü5 ¿¢ðš1o
Õ?ádðD¡?ÿº°?£Y¿è7Ïᗊ¿Ú5ÅaŸ¿ç<lݣߙ¿áʓÒ}'¿Øx\2/ýõ¿çÝu&Ê;UNASNone?ï˜Ýã[À¬?ƒ>¾®³PŠ?JæXÔ/×??4¨·‰?ˆ!œæ]Ë?'Êù3˜=æ?8ØR?…E<©A?UÁMž¤?]é
õW;?"ޟߦ;?ƒz;¸b?ïcÊì3*¶?®@±ª>N?dß94¡Áµ?_"-¬ÇX?ê»Y¹®?}ñÚÿ?ïd+Šê¡–?n֜ù…?S܃š
‰?<c×Æ_#?'<Æbƒ
•?m&ùžþç‰?ïE^n?‹ŽëJ]"?["ˆ,p¶ ?MŸqîÕ¸?•¤‹»	«Ð?Š¥³B"?îøa¾¿v? ³þE?d.sV?r!ÉT h?žmùÂIF?žÏOÏo@4?îâå¶ä¿C?ŠZ»É€xG?pcy:?fü	ÝyÅ?ŸŠjލlú?ˆn³…á¨g?îgجT?"®Äý?m°Îêb%?_©kF/¡?¬®u‡Œ=ö?Œbõ*XAGN4FGL J2323.9+2519?Ä!rÇÙÚ
À@ºç¯·éÀ:Ï'`—À<‡ô9rè@¢@ÕXå?üqišÐ?àÆdÓ¿/?ڒòK—
?ü¸ŸÔF=Ò?õÑ-=û¹¿èz9¢õ¿äYÈ]ÒC.¿ãEgéel¿Úü•½Aœ¿ê¦k93þ4¿ïýwƒ–"UNASNone3FGL J2323.7+2523?î݋|܅¹?—"kåÓÅ??mãÞÉeðc?e®¸?òX? I
HÎèë?–Dޞ‰Ø?îú\‹•~?˜ãiÙ×Û?€%ý1òÕñ?‡^
µ+?˜¡~}OL?ÿ`­EÇ*?ííàýŽê?ž:¨11Ý:?'´‰'—º?ŽØ¹Wtè?§Õ=o^ƒ?˜±¯ß
ß?ìÃÙØ	R?"/ˆˆï
6?ŽÄPÿc™?{ËË~Óû?¶§‹ˆ?'´áΰŠ?íÅV`VNc?¥	П{l?':…gÖy"?}vŽ«{m?¯øœóæù?£Ä0¯V?ìîŽ\4ð^?²7‰Q«?"†SG£ù1?š·öœ—	x?³iøK%¤G?­Z€ùë?íõíØ5?¡»±iÁ{?—-ږ?ÀÛo*nä?±ôðÒf´?Íè»È©?é¯"ë†e?©ø•˜!,G?ˆO¤•è?È@é,¾u?Ç1cK.,?¨tùÆà»AGN4FGL J2323.9+6219?ïÀƒ¸?ò"cښë©À:}Ñs$ºÊÀ;™®°'k@!!|o?@«j©Ø¬?ÖÙ¶Ÿä·O?µta%߸?ßÒèûV¢ú@®6Ñ?ïýä×Û¿î/¬*•ÕÀ¿È†ëA,¿ßu§·iŽ9¿â†=œBÁ¿àÄ(ï'µUNASNone?áO-?ĘçHŠC¡?ZWï·?wÑQ
›yÃ?ÝGª|Hƒ…?ĒIÝÞ[Ú?ÕfJ¡l?ÎÜRnM?ŽAï·Ô^?"¿m´PŽ•?äÓéëv?΂ŒLÌY?ä	õÍ!0|?²áoá¯ö?–-‡#‡?ŽÁVö&¥k?։;õÆãv?²ý¾82Â?è'õ´Äæ?¢ví£*=Ë?wCxÉ9?^ùÂïfù?ÎÉDGK¢?¢aoAèhñ?×HÆà?Å,þËx?d
=¯PΙ?e:ö(¨q?äkdžKkJ?Å9Ñ'²Ë?ˎ[~gZ?ňx)\oÃ?"C¨¥gŽ?"cÇZë?èË\Â8³?Å¡+֔ï?Ùoù0Ç·Ô?³â,ügŽ? §šëד ?"Ytß|²?â=‰¸Ðìl?´7qWxy?ÞÙ<
ï¤5?°q:'^·È?Þ吕?u"¢o?àS¤/Ñ|?°phåëÿMIXED4FGL J2324.6+3115?ÂÈ[Ó)LÀ<^ê–À:r®8(eÀ;÷|Gy;U@=eP@¿R%fÁÖ?Л™ðË/?ÒSû)×iß?ýu©dè·å@	Ñq§"=?íïMËdíÀ¿ãƒ!ˆZ¿êªó^1
¿¿îBÜ¢¨6¿ð?ïÿ~‹¡3UNASNone?ïëãº
c—?œr*`?Q$È0ÐÁ?‰7_±¤#ø?W…¤–a$?——–Çó˜??ïa3& !?"»0™Ûß?t8ôTY€E?€™èäýe‡?–¼Wz3z?‹õª'ŽˆD?îUªê­f?šUã¤ö—?F¸y˜B?ŽE…xW?¢¡­öYf?•Uei­?ïl¹ÔÍwB?r¹HÌ"´?f?¥¶v1Õ?MoÑãÀ#?A¡^T·!?p×o³¯(ÿ?ïêÝ+ó+?…ŠôÛÌ©m?ZŒTÝ^Ê?v®î7ÿ?Or¦°¨ðY?vS—ÕêÅÁ?î/´èCe?²N‰ºyD?‹Š€"Ç;?ž/yøæòm?§I"îLä?«©!.ËZâ?íÈÚR$À?Ÿ±ïÕ$/?"`ø¾f?üԆ½ds?©ÁÞØÏÊ?šUƇäÉ?íÖS*8Qš?•A">¢?'ãG#C?pòúF?­â
JÈ#?"]¥C©AGN4FGL J2326.5+8555c¿×n'×E²Î@7Q¨½#žÀ:²š'^À<1¸£J"@Ä5Õyï…@Vü9¡â?Ìu‹‡ÞY?—½"]?Ǥô^@LÓ±Ã\?n'§¯S¿éTký@¿é'^ÿê±d¿è›ÿ/p0¿ïÿ^Ê¾?ïõl=ÀÕÉUNASNone ?ïÛîOH	?kÍÒß÷ÿ?`Ó+P…½e?^sÍÏl*?c>µ;q©?c!³¿ÆF?}˜?LM÷´ËÝ?m–0L†½à?zX9ÖÝ?†Vi.†•?†^論?ï¤EçbG?ˆ:æÿ՘
?rŽ!h_ã?pEúƒC?˜Gîõú?7?…'BˆÙg?ïËðû'm?`ɦ>{
?O˶Whñ?9+/ðn«w?v'ŃÚü?\¼1>|jœ?ï¢è¿5yM?Bctêó´?xTJݯU;?wF‹:íM?v7U~¥ ?u
;Ríˆ?îÊÎQԀm?¨ìÐF€¢?{àü蝭?±"'½ó¼?Ÿ­ö'Ïó3?£Î¼üu1?í¸Gçl­ ?œM…èäd×?ˆ¥Ý¨Dá?"‡¼SV4?®WX—Ç?˜ÇÍ¥w?ï@,>ç
U?ƒ´2 âlR?j¨è³$:?]@¡\â?"¥[!lié?ù¾ÂÒÞÄAGN4FGL J2326.9-4130¿âê'æ›ÀPàñ€
À:h8:Ùð¢À<À>-b@D³'>0'@A–EQBé?Áy}Yò吿™hüe85s?ÒӌDÐ@¹fM¼ÌO¿êƒ
€òç¿ãz–~ÜÿË¿éI‰¶Í‡¿åç¼r¶¿ëÈorŒ¿ïÿûbâMhUNASNone3FGL J2327.2-4130?ïå:‹…ôe?‡-¶‹[­?Xƍ˜"p¾?†å"ÿ?\Ä[Ää¥?^áPG0?ïÙ/nM)?sü4Uy@?B ö——¯¾?P8"'b?q]q؄ñ?q0ž`ñ?ïw"ùÕ¡?…ÏJŸnAh?eŸöJ¬»?q*ÒÇÌ?ŒÏCõx<¨?ƒ×JO¿æ?ﮁÞÕ?b»ñ$öO—?H;.¥3;É?1#f^‡?'ÛՈó+?b#¿´Hº?ïͺ¦µA?t!yõ&ï–?gÉÐãA·:?jðxŽâ$†?j{‰?"§Q?e°rŠGR`?ïìÊ¥‡?ì>•¨x?V¤Ñû´?gF×U•÷a?‰Âxë64é?Œœª
Ï­?îð¬›:r?'	b:?r[xWoʉ?vüÝ(,x?Sž"Q
??ªÒÐ=?ïBhÛ5Æ?ƒM;Ogîe?dº§ ŒÝ´?U¦Ê…ýáê?œ]ú°U‹?'p_ »Ø!AGN4FGL J2328.0-2557?î	"õÖåÀQÕ_þmXÉÀ;V"tnÀ<撐Ü\@+È%Eá?þQ¶á¨üä?Û¾ó'ªi?ÐSX!+¯?õF‡nêÍ@v>Ôüò¿íº¸˜baõ?ïŒ<"Í¿åCá9Ñ]¿ÃžÅR…¿éñk}&œL¿ïøVž`3UNASNone?ïçª	d"å?VBU»y5?DÌÉù߸?7çsÕhüü?c"Ãðù[…?R±¥?oJž?ïâ¨âjvt?p4Äì?;6!ïÉC?HçñM_ä?iðYoä
¹?kîd°"pÖ?ïZ‰f¤,x?''ª…!ù?i~:…œh?g_DGÓ_U?'ã]éÝ?€Ìš'²Þ†?ïÀɋúŸ™?^ðŒÊo?Pñ¤u0?;˕·=Ô<?{^ÐӔ'š?]-- ¾Ì?ïÊnçFÿ!?n<]Úuß°?WòRSŸ?PÖE÷^ï?tËì"¸œ«?i$Ն1˜a?ïžBQÍìÌ?Le'YÝ­?Uô[ÇP?pÉxä«+a?…°à'ªE?ˆS~\pQ?îò?¥¦K?1&Žk/|?r̤
Þá]?so%½?󞌌Z?ŠÌG…"mÐ?ïzZ.t²"?wõwu^O6?Ví4cuA?S¡¹9!S?Ž‹ÍÞWª/?w®•%AGN4FGL J2328.2-4422¿ä‹V	÷ÑÀP€^"ð•À;£Ÿ}ß(ðÀ<ôy2?@ mnžÄ%ß?ü4 ½¨?×?(ßÈ'!?ÃCºió¹¡?ä{PÙ6h?üZËE8Ch?ìH‹¿¼C¿î:a?µøu¿Ïßü?Eö¿ÊrÜ@ˆ0¿æršA4Rÿ֓V¿)vUNASNone?ïyW2¨'?»ˆ[%7Š?Š_NŸëÑ?»žisG[š?m+•A\¢?kÌÜm¼?﷚ézØc?']@K?[š?XÎÏôY	°?bþXÜÁá?}þ×\ÚãÇ?}dFà;úå?ï^E<?€QKåm?ç?dÜg_T-?p½3{X¶?'›ËÙ·o?{Ï®óUÊ"?ï%Î<I?tÝSHüŒ?W|ɹûÄq?A¦ÕÒà#?™Îr_-˜?tqòSù‹?︽5LŠj?'Tw°™?NÃcâ *X?{ê·՛ë?Èøí3?vÒd®ÛÁ!?ï]ä۝†I?"šWV‹?b{o/è?qѝ†ô@?'ôâ0ËË?'c«~§–?îèéØâ?‹±sy 1·?j"55Ì'§?r¨]¢_ U?Ÿ¸Ü4[ÂÃ?‰ä'R‡³?í—4QÁ=Í?"'<•8Š+?c‹+$@†?Y´CÓç5À?²ª^7æ?"ˆo¢:­AGN4FGL J2330.5-2445¿ÒW ±.lÀQì<âž4À;,|CG}À<}€úfc@a.ŒZkÜ@™HUÚ'(?ÜA?Õ6ڇ rÒ?óšÞ¨—c^@I¤
æÈ?ïúy¾\òt¿ä '+"Ø¿éÖ]Ú¦ª#¿æñhÞë0¿ïÿ%¯¼ñ?ã'+ìíÕUNASNone?îÜ.¡S!?š
ΠÑ5?qŽ"¥ÃßÃ?hJÇÓÙ{? 
8ÃXn?˜¼Ýø`|×?ï•aß{?b*7N/?keF/T }?y\l­ŸU?ƒÎléD-?….Æ['?ît:<Å`Ð?•‹onԝF?†wÁÏåþD?o}ãnó?£k½ø¥l?'Üd})·º?ïL[<´Ñ?tÀ–e…?_("#RÏâ?H8RÓióª?"')ݍÔ?s18ƒ'?îyÒÎæÏÐ? ¾}Þåï'?v‹¿¸*Ï?r$qs:­?¥'[/<.?Ÿ ÷kbÍË?ïÓÀ(?£ª/ÿãU?yün¾¸+½?Q`3¶)·?˜ÿ"Ðށ
?œvD ''?í‹÷Pj6ç?Ÿ³›F™¡º?Ž&-QiL?†Bª'F­?¯¶ç,PiE?œ©‰C
°h?íál<FàÃ?"-"ó'H?kXËø)ZŒ?cɹן9?°×½º·×?"ËC,Fý7AGN4FGL J2331.6+4430?À‰Òž•NÀ0Q ÄeÀ;]ŒÁDŽÀ<À I·@ í;ÃO |?ý|s%³?ÑìoíÏ?¸N
áÀB?ê–>€nOi@Œ.'ã³?퐜ýç!¿í=äÒ}ö¿ÆÜ@WV¿Ù¿Ðºíý¿Ôÿ¶Äw¾¨¿å/uK¸UNASNone?ï,ۆùÚ?¹þ«Ô?LP'G#3?m6 >·i?™œä!´"	?¸Âf9™?ïMd¦Œ‹?‹Dþ3bˆ)?Y$Ì®'ü§?b}çÓã"?…ˆ
=á¯?‰Ó}Þ*¬Í?ïRǃóÑ/?€H?LW¯²?X…¦µCh¿?Pà4{Då?"µj¡?€5+ÌZ¹?ïMÃ#ÎØ?qþÒ%¢·?Q˜
i&_'?6ž¥gÿ
?•.²˜J
?qéQG…Lž?ï0'S­Q?£‹ô6ëq?Hå!‡·ë+?YÓíˆÚ?™3ór,Ý?¢o1>¥ýâ?ï¹¼"›? ãycM•?e"ÆҘ?x{-"!2'?šVcþ›ë?Ÿ*Æ+›?îˆæ/ä
?"ÜEl™üÙ?]âeVñ$W?Uº‰7{‰:?¦žn°'?"±®¢åÿ–?íÅÌM P?'TãaWÂ?c1rÁÑ	µ?U­òÔó?±8ÿ±Ñt?'"¨UÜñ×AGN4FGL J2336.2-0715¿âgé܅°ÀO§'`4PÀ;Š†‹ŸÛÓÀ<Ë+M‹¤@L}Dú0?ù>³†ªª?ßV·à†=?æƒ4õ«@àÎ&i U@þÎ4Uó¿îWS~WHç¿îùXG"©?êïàªÐ#¿ß2Š@ṿïÿÿ)@k*?î¸"†<ŃUNASNone?ﻅÿðn?…xíÈ¼-?jŸY†âèW?yn3Aÿ\u?tí‹ZÒäˆ?{—:Fˆ\©?ï­~>…‡û?‰f´é!j?`š[ö÷ÉË?pÆØSU?€yÙQÁÆæ?ƒ|³ÑÉvÚ?í/ó*ã0?£²ñÜáæ?Ÿ§zÂcÉE?—¢2…¾db?­-ìQå_?Ÿ{*fÞ?ï]x½Å·Ÿ?}
2F˜ÒŠ?BÏ-EL¬&?6p»kÒy?"ºnåá§Â?|Ã&ùC™L?ïdkyOš?•5Âx˜¿•?€ya‡Sá?ˆRÕSÈÃÂ?†kØ|»º?]­¯øŽ?ï> ³$–I?¡Ö2ŧ?nQÄ(æ?…Ù¨Àb?"aÉâ6?ž¦îLìp@?ìIø°
?«>"T²—"?Ÿ$@Xv?˜ÞC^ýÐ÷?·T (²"U?©Ýê¨ì"?îiÉ4g¥?—$¥{Ð?EKïóSöÆ?FCӛëË?©<ý¹2?—Ñ;zåAGN4FGL J2336.9-8427¿î­˜‰E°ÜÀ@.0Â?«À:ú..çtÀ<'äö=ö@Ձšt_ù@GÂÀð ?ÅsŸÊ`5ö¿ŒìMñz&?Çf™	Ñ»@~+±Ì?ïÎ5Lèæß¿áV8ñ¹`¿â´1?¾¿ækœ 1£¼¿ÖI¯áÚ{¿á,$€èȬUNASNone3FGL J2337.2-8425?q­8Õ?€×_(*Ö?F?P1è¨?5g×r"Ÿ?Œìî'–B?€ŒUÕÉÇq?2[ÇÒ?W²ž—=?b¾öåÂð?gØðs§`ç?‹MCºì¶?ŒÑ¨€q'Z?ï6Ê[Э¤?…ÈdίÓ?fvÑÍÐso?fXÜï"xÿ?–WÚM$?ƒü©áF˦?ï÷£:,L?xæÍ£
@?\·Œbë,í?CßϽ""?›5'ÙÂñ°?xä`0§Á?îõŽ¾ãïÃ?'ÌÁi`Nœ?Zm-,ÄfD?MO=ÿ,ý"?Ÿ§UQ½£>?'cïUÈ:j?î°d±ÛYØ?¤ùì'îÞ?k•NÓ_?v,~	,ã?£I›ŒZcE?¤·Q̍?îlà89'X?"y9ý§¶?rßl±
=?o–ná?¦ÖãUÂ?'•ÕuÚûù?ìê†ïGöå?—âbGÑ?tälpÕ«?fyhÛƒ?·]¼2iÂ?˜I\æ=AGN4FGL J2337.7-2903¿ï˜çóÍJTÀRiIùHUÚÀ;S·K[H%À<Ìzü ¯@Xs3©P?úØ»'øme?ÚÔ"Zï?ßwç˜*-Ñ?ú­êk|?öY<tz{F?ïK;½›Vˆ¿ì$2å/š¿ÓzcôF8¿Úƒw
S¿í×Þ
fðÐ?ݹÕcÊ)ÚUNASNone?íÖ&0|…É?«ÕӐ8?tEìߖòÙ?nXw˜™e«?°
o¬¡ŽO?«.',<4i?ï+¸PFœû?¤P¸Ãð$?~SY)K,Á?ˆWœý"Ù!?'ô¬U¤p? VjáC~?í.Ò·*?£àD$§g?·æâ¾?"µìÌ̕Ó?¯á™g3…?ž!\µÒN0?ìֈA¤Ýg?"rÖ
±?…w
‡õ*°?rcó†~@™?¶œÜ "ô?"tPÒ7?ì¨"Ñïª?·ºÖ¯h|°?†Æ|ÓÝ!?€¼ú¨mi?¼áïfÞ9?·SóÀÁ ¨?íô?›²‰¼?³2S"Œl5?"F:Õq" ?¡ïŠÂT ?§èÙB²õ?«"Ñ•ÇC?ì9ùÝq9?¥l6žq?Ÿé7¸_?•Ÿ%ÈÝ+?¶5ãQHœý?¡›Aˍ˜Á?èH³(ò?¬uv©ÉuQ?bŒ÷{ U?"¥5/ìê•?Íþvr?¬0È\øAGN4FGL J2338.1+0411¿ìúÄû$׃ÀK©~+VÀ;LÓî)>À<}3+¦w@!Ž:´w?ü/[7^;?Å1'Y4?"Ó= ¿4«?ÀÚA?Šb@§ákv¿ïÿÿ)@k*?ïì¿B ?î¾}=B¿ÖyV@!-¿ãi¬}Ãû¿ê!ۇz³%UNASNone?ïÙ:lÇî?w- HA±ª?+q÷m)îØ?!ÔÚÎã®Ñ?r‡d™ÏÍÈ?vê6tG±?ïáꜧ§5?q…½/‡©?6=c³IMÍ?C¬"¸Z²¦?kM·TŒ?oÛ?uóŒ~?ï!—Eg¤e?>¾áå~C?g˜¼[ñ4?vn^æÀíß?˜ÙÿÓCæ2?ŽŸS+›ñ*?ïP°?V
?xËSôFë?L}Jt‹Å?@k;³8¸
?•	Žì€x?xGqÂ.Ë?ïÆCmù?uÄ×u?<5ôž?2"¥g=?{øQÔi¿?uFÿ"Ÿd!?﨟‰ɺ?‡µ®VØ?GoBzÈKõ?YÑ؅SŲ?"a)œKǟ?†,F`à¶&?î 
KҖ?"}8K1=?g²o»'Š?sÿX¶¨9?¤"4K™Øð?"€Íb V?î§ÇJ›ž?Ûʺ¥+?Wf
àևr?VÒsì'ù?¤Ó2þà?¥è°
ÓAGN4FGL J2339.4+3008¿ÔºL[gµÀ>2É.4À:Ô®ôt±ƒÀ<Œt¬zFî@ Å#
F*?ÿ=GþœS?ËW+ lÇ?¨Ó7Â[|?à?3¡íûñ@°Ø–¯"h?ïڍ¯ãˆ¿ê¯À¢r¿âd2å/š!¿ÊU½â#K4¿ëb¿è¸¼?£o—ß҅kUNASNone?æ•\?vÇ.fÁê?QÉÌbÔÁz?A…Tšal¹?…¥ŒÅ_k?u$º»M'?û0Àñ?~}ú&og?Y_ìƒIÍ?\"Xóó=‹?"샗â­?zW}A?ïO¸|³¯Å?"¬ Š/­?gÇï"?k©ÆÅÇ)?"·m%X?ƒ.utNn?ï(*ÞûÎm?r{éݸ-2?hm"#†?KÌcG"mG?—ìñv#ò?q ¶÷Òs?ïI•r˜xÝ?‡è<#?_|ƒ¡ô%¾?P«°Þ´Ê°?"Õ‰x¨÷õ?†œÀ;w?îõU$¨3™?›ý§"RÂ?d®X_p?oRÔò‹ÒI?ž¿_obu?šèÝé`É?îå^øo#5?Ž¿½1Þ¦<?lQÕ:§—C?pf…ëÈÙ?ŸÉæI'É…?Œ¨ëìé?팤ä%ƒó?"BYÅ-?}‰ËbïÚ]?j;¸î­Å?±Â<(ŽåB?ŽÛj~¶ÚÁAGN4FGL J2342.4-4739?Ê?º[—;­ÀP[Æ?À:¤;ðqÄÀ<´;4‰tˆ@žÿãO›?þŸS‹˜O?Í)ß!Ž?Öû" áa"@Öt_Mmq?ýÃwÌ?^:?ç"ÕåzB¼?ß®3Äþw?¿â§'A°¿àáA=â䑿ïÿþR€ÖT¿®O×®¨˜UNASNone?é[c¸ƒŒ	?½JÐL¢ß­?¿øPo??¸Jô—'?µ,Þ!IUþ?¬ö?aê«°?êXI)Œá?Æ£I"e?»VCÕ(!C?¿pI'ï¢Ô?±çrÞåk9?´$öËL:?ᕑ½R»?´'Œb®³Î?ÑTÕýæu?±Å ­¤j?Çþè(?¬Úš¢¥~L?ìTo²%½»?"äþ×<æ†?°%ï^wM¢?'Ÿ/ÑA
=?ªm&ý»?…	¯^Û`A?æŠg]Ãf?ÁEÂh+Ì?Æû"XXŸ?¿ª"öiÌ?À¶R	ë™Ê?²Úc¸\‡?ç*ϒWŽ?ÌšÎwò«?ĊÌÊüñ‹?Æ#ˆ)s…£?½"éە+e?¼d¢=ò?ۗ×àÚ©b?¸FM["^j?ÖËïXñ?¶¥ µƒ	?̔ºkûY?±<R\<m¤?èL'o˜X?©Ç¡uQ?¿Œ¹ƒ¼/?¦¼þöÜ
?¾ºÿG?ŒÖ[ÿcAGN4FGL J2343.0-4756¿ÚBä˜Æ`ÀPR§Å¬À;b¸N†ËÀ=¥O°A@ ´ió
Ô)?üÇà"9¶?Óã=ñ?]ðv@>†TBw@²&|–~‡¿Ô×ûØð?Öß?–¿do³Âض¿ÃÑe¸Á}
¿é_9ìŠØ6¿ïÿü9¡â=UNASNone3FGL J2343.0-4748?îŠ;W;r"?´5º¯Mfä?ˆ0¬p'?™ˆ5NûÍ?¡Pƒýà?­Ó¾¤-*â?ì7Æ6Ê[G?À ¼ùpí?±ÈÌØ`?¸ÜpŽû‰?¨ò"º6È?©ã–'?íF"º ‹Œ?¢¢&'~k?
œd"í!?"*¦üìjÆ?­æ$‰7§?ŸÖTÁëv?êåãè™?§+¶ª0¥?¹'Ž k¤?¢‡ Ç?®©Eºó|&?™MRV)¦?í&܂øBq?°'L_÷Xß?ŸZ0à%?šÂ—X~­?®ŠÏØ?ª'¤(¡†c?葹¿™*?Ëêoïjö2?Á}\™€g?Æ4֒YšŒ?¹E7Làgæ?ºmãMÓÚ?ëza˜ÔÖ9?¬±Þþ¶Pu?¦!¼ƒÜ÷?›ºÝñi7?¹*Ùͅ<?§‰]ý°F9?⿲O%¶?¿cØJ7h?ÐñºøŽòw?½a78·'º?à sE¥"<?±aèô½ÛAGN4FGL J2346.2-4322? Ö%QYHÀQDÜ3rTÀ:ÝW4šÀ<§JNØ«'@ýG#Õó@	q"Úí÷À?ü]ò#žjº¿¤¹OÂ`Z?ؖ;`~Dÿ@…ê⣿Ò`£üž÷¿ížo÷ß ¿âqáÄ«–¿î©;,ü¸M¿ïùL`RP?Ë,b^™éKUNASNone?z=wŸ?¥ó5g!¤?¡È=L5ë?¥{ÙB»Œ??r]2†H,·?}¸{·†?ïÉK?Ûý?‡&tr"|f?U©Kú
§z?s#ÃÜÄD?uð
=.?7½÷žl?í¾<‰J"?¡½IßP?Ž¤àæ–?'fGØgÒÑ?¬rÿ8ö9Ú?Ÿ%N¤Û?ïöÌ[ýp?OøP†^!?
¥–çüŒ±?Ÿ‰f—?Q'F: ˆ?N‰=_ʆL?æ(­7?£žeõìðs?xvpCçºÕ?"Ù•]éû?{¹œ–"´? ÌÏD)`?ïk\<õ\l?¢%Xï¿È?h
ïnš·Ü?ˆ«À~.?%tïñ3?þD<e¤?í°>h4`Ÿ?ž§³¶ò?X*º`?"¹¡•Ê(Ä?°SeAPÂ?œª/õÙ9?ï̍¢?…|?'¬ÌJÓ¦?1úaÊ–Û?f2ÓÌü?x™ˆ½¬[?'cÕ¼<ÙAGN4FGL J2347.0-5720?ÕOJ×oÀLÚðZpŽÞÀ;‹¥·µÀ<ã?«çy÷@ö¨M'ƒK?ý ìt2?Úy¤)ëa?Úøäl-P@ y¢ƒM'@<!Gxd–¿ïü£ŸVòÖ?ïÿD¹mtx¿Þ¥¿'6{'¿ãkŠýõcÅ¿ïÿöût€?î÷ôÎs•úUNASNone?ï¸_ùŒ?w¥IÓù?aZ"½éz?^
­•ïô?{"¸û(f¼?s‹Ñlˆ+@?ﺲԆ³?}²gÿNG?Vôæ¼K?a	C—բ?|é\Âû¡?wÝô˜p2?îkºî‡?š©veÊЗ?"Źx«94?¹(ûw?¤gžÛÞõ?"vw%‡kG?凌F+f?g+à—^q?[yU'äçÉ?Fñ.á\)?ƒ+ƒ¶‹F_?dâ›ôóF†?ïzèà9ø0?†Ù
K7ÎÞ?sÙÃ"´Œ?sקseœ?‡XæhWÁÙ?ÍºË|òm?ïDv²¸'?˜u©×Á?l=Õl'JV?€žÑ¨…ðò?"éƒuz?"#ÓÜÅð
?í/Ô5™6j?¡'—'Ÿ'?›¬£ŠÔÇÒ?'Cýo|Ɨ?¯,jܶ²?œT§"'Ý?ïƒ7ÏÇu?'üÉ+87?c|ŠxìÐ?\Î ªÕ,?™À»ŒèÄ?'Pۄ´{æAGN4FGL J2347.9-5106?¿(å–6&œÀO–/­lµ5À9£OÄcq¿À<j1ßv½@s€Êë¡@¢%ߍ™±?±X¯ïqgv?¦î2ß6—þ?òDÊÕ{Ç÷@"_õ3d¿ÞÉë¼&6v¿ä&Ë4*ª¿æ`C¢?Ý¿çzȞü·¿çQ	<¿£ï¿ïþ SUNASNone3FGL J2348.4-5100?ïù‰d©^?>µd›lB?ÏßËßìT?XȏҠ(?FqZÿØ?;¼aóûf?ïïÝ<ÓèA?e
Òo.Ò?*É WÃ5?<=A9Ý?]mP.!l?bœ.å͟?ï÷;k?b2:Þ;?R'ÝS2M?<—QÙE]#?yÎ\Ïxˆ?`µµ†¢Ž?ïöÅmB}?5©ƒp͋?,"ñIDö·?_‹é"©½?MÅx‰?2è¬×öMG?ïñªÚ+&—?Rø¿Iw‡g?-ìö{å5ü?#ñù S1?Xì¬Ó•p?QkÿKAu?ïÎþøäû?~¢»"ˆ¾ ?;‰Ž8"}?P[³Ke¿?vÈk¯÷?|oZNª°â?ï–Ý ú?sò¡%‹|?^—vúiZe?QÕaQñ½²?†uÉ¢ú*#?rê
ْ?ïèeû·=?T×n;û
?C|³I…†?4Bü¡ÉQ?b»½ÃOï?RR?]¦îAGN4FGL J2350.5-3930?ä†]Uh	ÀR.bÀ;XLpñÚ£À<Ç$'&µv@ö‰QLù®?þºƒ-?ÚԎ!ÁEÛ?ár×Ã Ô @҉T§ø?êIWÚ(ø>¿ïHðŽ?ï`?àÓ¿ÍBjCk¿èé£Ò؈¿ïÿs+(x?ÕG$ARۚUNASNone?ï·¢yù&ƒ?ˆ\E83ò"?YNH]Göè?d	¨HE­?}Û0ìʬ¬?…L_¹‹?íÓAŸÌR?¼-Rê ?¨n ¼Z†+?³·ìOèÙD?¥ä«-Pª?¨ò—ÈÅ<q?ë±ÌÙëvå?§{Íð}?¨*ÖW
	?šþá˜ìU?¶\.±P×?¢žX×BÙ?ë..&·'k? 0`×òtñ?«2Áƒ¤'?"°¯6™,'?¸õ.	M'¢?˜:S,½??ïE°–éĈ?™Ú¿Øa¥?up-"L՜?~óÕôïxÅ?'íáߔ•?•ÏœÍÌ?é·=À7?Ȕ¢¤Z<â?¹`"Ñt ?ÁR
BÖ?¹-±jbø²?»ô¼Èü;X?ëIäÕ?§¿ÅŠ/»§?©o_ã}Y?š®I#ì`"?ºN-àc­?£v[ÜÖ¢?çy&l=?°È÷à^À?®OÔ¼uà¯?£X¿c÷"?ʇrÁyâ?­"Ðˆz*AGN4FGL J2351.4-2818?æú*ÀS+à`þG™À;&ˆ|:äÀ<¸¾ aŸW@XŠv;³@ä®ZZ?ÏÆ_u;@?¼§0ž-}?êŽSz
ˆ?÷àO"'é?îa.¹Pï¿æúf=v®¿ã.^œîc¿äîV,\¿â«={
¸¿ïÿþøþ"UNASNone?ïĈ†)'ä?q³8/&H?9P-®?+?.›×õ¤?|&º'uÕ?qc–ø\w?﨣Y®>?ƒ•Ï}"?`·ÖQ£L?eûŽ{W
?©4˜Ã?YÇü`¶?ïKKšê?ÚQ¢<\?p'"/‹U?pÜÐH-?'xï*Ùñ?~Aü}€:£?ï,)žßԑ?sjAyáZ0?mŠïå
u?Rì?1à?–ÉnJ?Ò?r¨Xü&÷?ïz[Rƒ|ï?'î{ACÉ?L
@¤š²~?A£xÀ—¯ ?¨WGpŸ(?'œ»˜¸N?ï "ðȳ?›]¹Ëfñ?q²ÿûZL?€d]Fßè?—'¡é÷'?—P¿R—¦?îÖßç?&*Ùiá?|½ä ªº;?|ÜõØj€?ô‰îð|ï?‡ìúê—c?íÍ8SK×?õjk£Ç?}Ï8j0F®?m•¼ßçN?¯r˜ª¯Œ7?HBØÐbÅAGN4FGL J2353.2+3135¿ÓjÆÐÀ=ªV¼¥7]À:Tð=ëÀ<JHêT@u1æ,@Ø'sâP?·ûø‰iÔ¿§¿6a;a?ív+57ð1@	WS\¬ÿ?ît=¿~0¿ç2–À¡E`¿è~=½Ð°‡¿ÞV`x»þ¿ïÿþBe«+?ïÿì´É ÈUNASNone?ïô¾ŠÙ|?PÏ0Oä#í?>Ø@K˜Ã?7E*G¬7Æ?PUÏ;aœ?K|›T;ös?ïÃ~)H?zÔ¯Üqq?OÚúPÊá?Y5Jÿöwn?z{a·3j1?w&û×þ4s?ï¸íÇ:³ý?t‡Ý{~z?_OC÷\¥?eDå(‹~í?{µK~<¾?q®WC™>ù?ïØ)y¥€?T"HÎ-P—?LH?ìð ?5@nÀx)?pbj*Xª¤?ReAØÒg?ïë{Å¢P?\áÒà§?M™õÞ{Ž?J±!lÔÐ?Z<Ìž?U¥PD®þ?ïOÅ&݆Ñ? wÍøc?[ˆ	Ìv?jj¨]?"Nڍè{ù? "D²?ï‹}Ö´F?~|*_{§?f™ÿî~͌?oz—ÁÂH‹?‡z
dXÇ?yM÷h,"J?ïppg58?xJøÇà}{?mj$™	úF?`"…ž''?Œ‰]sщ?té¡f'fAGN4FGL J2355.2-5247?äPS]'×ÀO#ãŸw),À;žUÀüµÀ<ÁÐ%Fáf@‡Ü¥Aî@[ˆ^Þ²¨?ɕµ‰dBJ?à…°ÿì·@,`RP/@
.'uÏ?í#P!U*¿ÆbK#¿Í¶¿à¹*ù¨Íê¿éþqTÖñê¿î[ÛÞb¡`¿ïý󀕼•UNASNone3FGL J2354.8-5245?îøðÍe¬‹?™r"wÈ:K?gž¡u˜ú?ì9K;—Ð?zG°°?‹"ïÜ*êŽ?îÛÌü6`©?¡0ý´,_2?Œ+‰Ÿ
#?"$žoá\?–pÝ-…-Ù?""­äŽ¼?ëÁ\gp8?«£œ'GjÎ?·CY9¢Ñ
?¤ÑÉ¢%"\?°®›äk‡µ?¢³ÇãÇ?îiw2;'|?…à™.ûñ?–Ð`ƍoI?wŽCczÎP?œ¸÷'Ë=?€óÀ'½ît?íéôå½?§|i½Eá°?¢QŒ'7ê? ãþCq­?žKFY¾~?—»hòô¨?í9û8gq÷?µ€È—÷Ü? ¾	9ÔQ?©=|c-ï?«¢0m»WJ?ªšÛŒMï?èc<T "?²·]EàœÔ? ('Mþn?­­ À?·¥ÊZÙ?£3#9ˆ:`?ë7#"¢tè?¢ãz‰¨?°LŠ·l?–zøÎñ/Ò?µú\Ø$Ò?ž"E¶SÊ¿AGN4FGL J2355.5-6614¿êD\Þ¨A}ÀHøSX"À:]RtA}À<Zºà;>š@·Â«ášº@†÷ µí?¿¹? §??ÑO9c£éT@Ñ ;tJU@"é3_ÓÐ?˧9ÓtÝ¿Ýë®ÄùäFfގ–¿ê–—Péý_¿ï‰nÿBž¿ïò
"þ2UNASNone3FGL J2354.4-6612?îvðYL€? œgÙº²?ŒèH´Ã¤?Êf'œq?¡d0iî?˜hKÖ©?î !©P¤f?©Íƒàö?ˆãû92*é?"¥ë'1­?Ÿ‰Í7šÓ?¤&L$XÀZ?í´C`tV?£±úðháª?¦Ðû?2 a?§"+Ç^Aâ?– Dw‹ú5?îmÁëáÿ©?€˜9X€–?‰~¬i'?i"uZ"ŒÀ?¢ã¤È 
?{Þ…òÝ«?ë(ôpTѾ?·ÃxaKÜ?©Ñ9òSÀ?©S¸8ìË?º+óßòT­?°Ý¤Ы.?ìúÚÇaS?µ é¤[Û?–©ÀªÀã~?¡Ù\@?²~¹›üý?±N¨®°84?é4"ªÛFž?°½
Ð"?ºÜÌ&è)Ó?§Ò؆g®?»'=¡:?£×¡õ°1;?ì0'?šÂõè·Õh?œ"Œþ;ëÐ?†[£1 s
?·^¤N%ç?•Ä|,/AGN4FGL J2357.8+6839?Ѐ²Y¦[ì@/çáüúÀ:{·0ƒVÀ;'²´ҟ@EóH6¦@
äÏ©?Çw¹…_?·oóegä?ñØ·lwÒ?ÿ$SÚÁ'?ìÙ]ÔÇm¿à²Åº‰Ô*¿é…¡êöÙ¿åá';"¿ê8'üÕ©¿ïÿèž:UNASNone?ßO6€çéU?¾Ùñ"—"–?‡à߈¤s?zü:µñù?ßñƒ%l?¾ôpL:¸…?ã»÷É¿jþ?À{́DÛt? |ñÏùn?˜úÌÁ7ù?Öx~®~$–?¾âuÒ%bv?åþeÂì=?°RÊç? 
Q³ñ2?íZsÚfj?ÒêIú
ç?¯7ßÑrŠ?揄‹{¯à?œ3Wrã?¦:=»á?R°Ï‡¼s?Я19 ?šO–4ߞ?Ñ°ÂÅ.?ºütìLU)?•mNl\?‡H˜?©?æ|Ž‹ÉwX?»¿M®ðª?Óý€Þ%©w?¿YŽkŸ?«í÷ê²»Õ?ªâkS?äB`Aÿ‡?¿'âêgß°?܌´'Ë!°?²ó!5´á¬?«àWÏ6îÛ?–NY/8€?ß÷@t w?³®%EH"?ÚÓó"qG§?¤üCƒž–À?µÆãFkÎ?"¯®/‡)?ߺSšÔ#¦?¤èÂ9µ~3MIXED4FGL J2359.3+1444¿ämó¬KÀG ÌݓÄnÀ:ÌhfçÀ<tlâ˜@êx»}š@MvûßßÏ?ÖÒ~ýáí›?ւ[Ü®l@` Ùÿ»7@rX¹TŸê?áhÝ{µƒ¿â9
wt¬¿ãØîª_å¿ì$4'®ÃÍ¿ïèè¡¿'â¿ïûÕctCŸUNASNone?ïAÞȳô ?ŠÅúŒ?d²Q€	''?Z^JÐû?•-ܸüV?ˆ÷Ԗ"Ï?ïY|\? —'`ù?q
ëxÁØ?t{R>°?šÝmW<?ˆ—Ô¢'^?îæυ
ñZ?'I\UÆz?S)2'iV?~gÝòÈ?š|zÂz?âW'#Ž?ï¢:8FT?uH]«ó‰ˆ?uÄ/âÌ3?YëÕT'"?š¬ÆËj?r§ë¸"Žv?îD±º¡R?¡û:Á?rû—'é?k/²Õ¿·~?©UqzÛWC?¡#[xòf,?îH._kq?§^†…+'À?í³_G?Ž¦9M1?§µãc%?£´¿ø™}l?îůÍ¹?›ªñõj´?Š.àñ¥|Ú?…4¦Z/;ü?¨GìÉYŠ<?—Ðƈc\?풁Øç¦?'' W)Ç?–îJt8#?sHïmð£3?±9ug[?'?Ó¿*-îAGN4FGL J0429.0-0006?ï‰<"€|À?BÝHE0À;*šÞ=8À<!-••@j/Úc8_@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ÒûÏ×g?îuU9y¿é‡V +à¿ãý…Â!M-¿î0£kªs¿ïþx«ãH9¿ïÍ®5öAGNbcuTXS 0426-002?ïãŠ^=M?j&Sf-€G?:׃lÊ-?6#™ˆìœ?i±oÃÄ%?h§àæ™?ëûˆ™?†	;2É…?a*~³),³?sR;ô'Nª?"F%MtV"?ܦ>W¦s?îù3C­æ?ˆÐBÎÝ?}Ù×qsdA?s=AgžÏ?™c*•$0?"è§(5nÆ?ïã²|Ù?~
k=ŽŸ?XÈLtt´n?Cc>ÜúÊü?š—Áå("?}5-/X?ïÊ(<à9?y?"<±ZW?CÄÚ8w|µ?BÚæ$"†{?xsFkm»?x,"­?îτol'?¤2ÒA)5Æ?x 5zۅ?çâõvP?ŸçdÑÜn:?ž@š`$>?í¬ÃXÅ`?™v%:
ÿ?~÷ƒ°?'sU·hsÉ?­TÂâ?•Õ€ï?íŠÛ­p?žþd¦F?jŒçïÙe?`»/Ô¡‡ñ?²ÚÌ9Hö?žT³ÀÊ%¢AGN4FGL J0534.5+2201i¿æD&v|cÀ <Ž%ÈÀ5ì"ÓiŸÀ;˜=)HÏ@"k±»¤[j?ü?ȔhqH?´zá?òõ†@íT¬ª˜?˯¤Gó_¿°^WàL퀿Ð9–m•/¿ÈÙ
¸OgF¿Þ:—Àü_¿Åa2àRÂOTHERPWN3FGL J0534.5+2201iCrab Nebula?ï5øh9®?›‡çUê6M?&¢d}?'TÆT–ùq?™0¹…X€?›rÍu}?é?4ÙP"Á?ÑBknd?§b"–Fê$?À÷"©Ö±0?Å*‡µbð2?Ìh›?è–ÌÀb†2?¬H€‰h¤"?–
ðEýÚ?'ì­¸–|1?ÊãÁ¼?«éÐ7?ïäüh? ÊŸ_Ém?™ší–@Ö?žM,'[~?y)"YåXC?|4¸»À,x?î,œZ?©41뉝?0;Ò¼—tÍ?5ÿD,Ç?¦ÞUº?©#M´(H?æý˜WáO?ԏE_Rq?§\0 'í?ÁëÒ(+m?Ðç™Iñd?Ò¬hÜÀéG?懻Ì'?¯°÷íO?˜‡¾s?'õÊS$/?Ñh†ÿ–¬?®´a6g?íàIæA׫?»6eBØu?©éQQ
ý?¸ù¢oùY•?$!9¹ô©?žB)(¢AGN4FGL J0850.4-2558?ÙܝUÌ÷P@&Å«ŸU›=À;CHdàÀ<Qpنïs@û&s\æ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ùwy‰-ç¿â'¡Ã3Æ׿ìªÒ ɤ#¿æÖ¡aä÷f¿Ö؉™qV¿ìŒ$ÁUuR¿ïӜ_F·tUNASNone?ëëNwSÀê?¸+ÀÕ^?'"']ÍB?Ž¡A_š"?¼]&'S`?¶‹",¥?ë*ôgñUî?À#B@R'®? &
}8‡? T{Mkÿ?¾™É·òÎ?½¹ŒV0?ìþw6Ã5Ÿ?›{¤9{cÞ?œUøåÕ?‹ˆVï?°öÈ+¤ßÎ?"цýª<?ê3.ÅT!?¢p–lE?¡Û¡^ó?ˆ¶3C©l?Û|ƒðK=? #ŠuL?ä¬yd^¾?Æ<ÆðaI? ÑZ†Km™?–eka=?ԌáæˌÂ?Æ<¢óŠ?äz6§ÜÓ?Í•t¾:Z?¸.%êÄ?¼Â,›û"×?й'JÑ4?Ê<Ý'û§?élÃ&Þ?¦Ýs#"L?®,>7ÎAz?–óú…?ÂÁãøëí,?¡hÒ '?áMpÎ?³ÎM-±ô?µ4_û`?¢«ªç
°?ØUR9U.?²›Au9i¸AGN4FGL J1039.7-1540¿³0TzüVš@BKl6KìÀ;/æw˜¾À<Zíl…@[öëYTÛ@θ`?ÓÀ–?"aï?Ån¿³è-?ñéÿ¸‡p@Âë'D"X?íãC ¼
7¿ì'lá)Ñ
¿ãÇ=áâއ¿ïŃAéYu¿ïù™ê!qj?î"Nü½UAGNfsrqPKS B1036-154?/j·ë?¡ö¦±w_G?J.oTð|?G°¾0ª)?Œ;")?¡íærÇ:?ïH˜ä³k?–‡gªî‡†?y·ê}àL?ƒ¢¤µ¢}à?ÞZ?œ?Ž¶ê]7…×?îí3«dX€?"L¬¡ù*t?|n,ÿ͋%?péeg†¯?›=ÿW$&?ZaÌSû2?ï¨ä‡ ë?g÷&'!X?Zé?ژŠÎ?E3W|Ö?'i¶¢µ¬?eg
Kå/?ïWÝSŸ²?˜™z®Õ'…?V-:àK'?S£â¶¦p?"¢'Ånhü?˜-ÜúDéº?îXY<?ª¯úoâ?…éHýv˜ ?"ÅO¢L?¥Ì¾?£É|Q³qŸ?íqXH¢J?•Î$òä?{F³Öw?€êòº!?°…Ý[,¤ã?'}/ l¯?îÀó³Ÿô?Åã/¬ï?q×£&Í"?e—J´*%Û?¡µÐ^Œ.J?‹5*†1AGN4FGL J1202.9-5717?ÝÍt
•e@ևà3±ÞÀ:å¼dŸ¼ÉÀ;É>adžæ@W=Œ¨ou@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ZRúMäd¿çëe>H:?ﳫ=°å'¿ØÎªžœ¿æébßôñ¿ïÿã_¶Hý?á±À6UNASNone?å1?%ðz?Äþ]dE`?ªØ'u/yb?§
‡éÿô©?ÒBogR/ß?ÂÊ$ èû?ã.ß^þEÉ?ÅhÙ»Ñ/'?¦V"ï?©§Àù?Öß^—1Ð?Ã1µU.R?é͘tU'Y?¤_e£ðK?¨Ãû‹ßÄ7?'›9•J?˜ŸLû ? /Û˜Š¤?çÈíõfsý?§ê—ä½Î:?Ÿ7Þ­c¿²?…¤n—‰àC?ÌõLT¹¸?¥ãŒþfÞí?Ýyݚ-ô?ÄXXPùí—?¸ÇÌÀ4?±úq¨;?ÜT/5ç\_?Ä!®{}ú­?Ö¾ß8?ǧ½DÇó?³Öµ¬:T;?¶¥¿¿+?âIڝ"™?ÇHŠGìþ›?âi䗑# ?°iY \à¹?ºA8óZ?Ÿsõ5Ŷb?ԛèÎàù*?ªþº²MW'?Ý{®ˆÝ?¶RdÚRÐ?­0EZky?œI^\›{5?ÞÞITX±?µ}B›qTMIXED4FGL J1209.9-5923¿æŒÀW?ú8@o¬)ÜrÀ:rrÓ\3À;<¤'D`'@k$†r'@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ø¹µ‹g§¯¿ï,,À/[?ïõ0~Mù¿ãj–â/4¡¿îÓ¬àsGË¿ïù'm-*¿éê•ÀF+³UNASNone?Í8ídû`?Âm-µš×?€éÜAÿ½²?|#!Èõ£@?è{ŠSÅ=Ñ?®2ÒT?҈IU›?ȽÊא[?½¾'1aÔ?ºy"N>Ò?ãoOƒ?Ç÷½å4?âr	÷irN?­-‹VõU?°ð
ª+ã?"1\g‹´¼?ÖßéŒBk?ªúTz?Nj™¨Gv?¦Î[/`È?±ß{–h?—j¦…óñë?çüÝË£Ö?«c·L—d3?¾v{OŠ4?¸ôc<ÓV?'QÜZx5`?|øi¬Ã¢?릡³¯õ?º6l§âÌW?À^Œµ')?½Ž'†¤ì«?ÄSYEö?Ãæ€Oúî?æӆR¿¯?Åȝl.t?Ôæx3\=?«­µõÄä?½A¸¥+%Ñ?ã({@µt?âTÕ¯Ê]‡?¬—a—/î?²g[<_? (6
@/L?±"D"ôƒæ?¤4a/À˜ÿ?ëŽÔcïé‡?¬mQ%MIXED4FGL J1320.5-6256c¿±åg'2r9¿Ð¥é^'þwÀ:Ĺ­À:ÃM~8D@!XÒTÌ
/@…Áÿ¿=m?Ù6>`7ù?ÑìD`Eÿ­@=جÔà?æ€á;ïÿªÛ
}2?ïôßÀÅWŽ¿ÛàY¥"¿âr·bWc¿ìp	è·UNASNone1FGL J1320.6-6258c ?Ñ3ãöù¶?Èf¤Púó?•Š-ž|`?¦"­'•Ø*?æÌ¡UXU?ɑÁ…Í?ÇžEÊ&?Ëíq¢Íö?"GÃ?¿æ? Ì'bæí?éžZTp€Ø?˘/v»M?ځ1{֘±?¯‹qŒÚûV?¿bŐ &Å?¥þ~í
7‹?ݦ !]ž?°L¼ªTw³?Ò š·Z{?³dîÌcâ?yJ)\®Ki?l<Üfâ$?æ}RÌ£?³º›Ô;¾ã?Ð)I/HíÛ?ÈHÁËøø‹? )4ëdÕ|?®ø|ñɀ?æèÈE«?ÉÄó§#'N?Âʟ>&ßÆ?ÃQ[Ÿ/}?Tëdž'e?¢Íµ<"Ë%?êÊ°ÕlÐÛ?Æ¥pm·?Ð?>ÍMÙ°?¨'×;CUž?ÅúIF?­"åº5o?âž\ÚÕÖ?°Dþ¦ëe	?¾<À¿g"h?¬&¦`
?{™@˜øe&?|÷‡oMPM?ì5g@ ?¬þ)È´¼OTHER4FGL J1622.8-4454¿Ö9=u£½@
ß_ü¿ÙŸÀ:?íë*…æÀ;I6_7ü@³›õ>…ø@uuf͔?ÔÉ@v¬s?Ð~®?þ'U_­å?þìrtf¯7¿îîoÜV?ïþê‹út¦¿ë§žªz'm¿ÞJû܄е¿îñƒ€R ·?Áƒ-FŠ(
UNASNone?ÄÅꉺî?º9÷ ø?´impµ?‹3C¸â@D?êW³¸ 9Ô?»¢ðOe2?áJgaO"?Ɯþ­3n0?«•f?$®?¬¦Ø…2q|?Ùø… Õ|c?Ä~`t?X?âß:Qy^?®'ðÝíf?®¨•cÛÆ?"–ÉØ(»?×ë/Øy˜?¬Àæ€ Mˆ?ál|nKÉ=?®"2J¬«Ø?£†aÄÆ7?…Š!b˜~ü?Ú¶:ët"â?®`Wˆht?³àéƒI™?ª[EÑ ? Øä–IJ_?Ÿº¨áI×F?ìvT†·?±{ÅÖàã4?ÒøüðE?ÄJÄk̤*?»	i~)?Àf·f'?ã"ÐQ'¹?ÅÓà¡YÆ4?ÒHix è?¬ÃŽHÎ=?½V•ùQ<?¡FL	€Í¿?ã0ø…Y¾?®þ©Ñ¥?Ò
L™$˜€?±
¹EW?©.bãUù?–|äy‰%P?ågøh¹°?²mƒ~3¾MIXED4FGL J1758.3-1920¿îpÐ#]A@Àó°fÀ:³!*3À:Ì&€IR@!
²˜@LÌ?ß ?ÝF"µ…'?È5*ÀY22?úâÿýPÎ?þ3³P¤Þ¿íß/ûÆ?ïäÈÁû7™¿æ>Ê€Â2¿æû]U¹¿è?tŸ&ú¿ïÿæ4|ßOUNASNone?Õè)`1Õ ?ÅÓú~
òÍ?Áû×ä\?½ÛÄvçèÝ?àŒõŽâÜY?ÊTÉÛÖ«?ÍNóŬiw?ɧ밬u?·ÿý²»2?ºÙç‰ÞÝé?å¬CX"œ?Éÿ1)~åŸ?Ø]ƜS¦?®æEµÅ¹?¼Ûïêß‹?¢œÜ–¯µ?à5žµÏ»?®Ïþ…‰­?½¨Ü¤þt?Ÿ™aü¤tÍ?¯n[6Yÿ?›¨¥Ù¡z?êSþ·Öp?§6¨Cµ™?эæ"CO?Á¸›eÅF?ÐqC°âi?ÇÄnré?Þþ¡ÊÚH?É4Øöb»?»¡Ì\Ô02?¼#~à/Ö?Å)I$Œ&i?ǹ©{Ü<?çAt+Bp_?È#QÜÊ#ƒ?Í>KØàE?¥È5¤Û?Áö_| ?¤øüÎĵ?ä2÷B(ç?«/í®n½Î?ž€dia?ŠSÖ8Gj?­ö<¯I3o?¨ù@"
®?í,™Î"|?ªü
¼ˆgOTHER4FGL J1838.0-0516¿~³¹ì¥y?áöѝìåqÀ8͘¢ù"¬À9ïœp
¯@%¶Ê×Õ@3€*?ùCO`Š7?ÖÞEvX³@"Jà£ï3@K¹•ãV§¿èîVŸÉß]?î8†ß'±÷¿ãý+-«4¿êÌ W"ý¿ïÿšŸ¨ý:¿Û
! á÷×UNASNone?Ɗ±_îŸ?┛i8º?É1Ëv'à'?Í ÚÇr
?äàâGL4?ρþ™á6?´àH µj ?»L…÷rµ!?»f³õy?¿û&ÞÏ?é÷5å{U?ÃL*oY?Ð^°B0/?¤9/Òy¶°?Şc¾|Ž?¥²}/Sö?å´gúÿÔÑ?­PŸ³A¾ð?¯ëÀ'ç{z?(ú¿mL?''8ûiÛJ?œk­#g?íl²/èzþ?¥…÷Œz2‡?³ÔtšˆaK?¸¯f«"i?ÆÓBª
ü?Êp×Õ$ÆD?çРÂ`j×?Ì.재u?²íۑÌ÷?¹\ÀBé?ÇëÆFœ5?Éô·3w@?ç§l}ל4?Ê_±ð—F?¸ÚÓþµÌ,?–à€³Ä"?Ç?½Î4ßc?©5´HÅ·?ç¶ŽP2?«ôj(Ew?£Ýê¥|† ?¤f'+nÚ?
õ¢^-@?¨³Y^@'7?îA±¨Ùþd?®Ô›¨[ŒOTHER4FGL J1841.3-4442?â3mƒn½À1R`õäÀ;R`îWaÀ<{y¾Óæ@½›yÙ@¯¹À*§ô?Ï;˜@—ä}?­"@ fäÒ?ßrl@gpŸ@
Nܱò+?ê…cíbt?ï^JZƒÚ¿àiPüqÖ¿æÆÙmÄÿy¿æ˜y¾²Ø°¿ÅÁÂ<1µUNASNone?ïŸ&è»Ú{?®±åA˜??‡±;]î4?> ?¬7ˆÝ?‡:V¿!?­ÿ/	RÆ?ï°½Wcê
?€ã•;"
~?X1߅î?g:7ãý ?€Ê‡†õ7²?{›Û6˯É?îïU&¼Ç
?ß
§ít)?w("bîñ?d¶	ßUx?œTÐÿÆÑ	?{á
7	®4?ï-t´Õ+¸?t'ƒ$ãX?p#ϱι?U˜öR?–Hu¢‰üD?sŒx§E?ïƒo©¹ªå?†÷U<·/?QÿóÍc?EœK5©-ë?ŒôˆtЄ?†–UAzô"?ï1ÕW,Y?˜BqsóˆG?o¼¤¯b\?…zô½
?•ÍÔ ãC?"ø­½Ö?íË"SD©0?Öæ™6#Q?†oêeèPÝ?t5-ÅqJ?­±à/§£Î?ú¹?íÈ<ø·ií?'gð^ð?€¡¥à,ƒŸ?qbÌ<ª?¯SÆúÆrO?'^Ðr:§AGN4FGL J2048.4-2517?Ðq˄xJ?ÀBa$FEÀ;ž6a»Ü»À<Œ~å¹,Ý@rEêE@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?üŒ ŒÒáº?ÌWµž‡êð¿î·Þ"ž­Ö?ÁB‡dð¿êj˜Yþy¿Ðæa=²"¿ïÿÁKJ‹UNASNone?ï(%¶Gû?'²}ˆodb?h™ØYÎø~?f²L­%'4?—è"«Ç1?']-¹"ãa?ïªv$ŽD? Ùø«ä$?*ð+?©ïvF¸‰?—¬Ë¶³l?•Ú¢¾Õj
?îã{m'2?'{(3]¢?Ý§5o•¾?'j"û"–E?¦ª^|¦Þj?Œì¬óó?ì.T#˜¶p?›nÏ~sq"?{½{üȹ}?oAÄ)òÕ?¼Ñ‡$T¦©?šÒ_Lí?íÈÉjl°W?ª¡}õ–s?{Î0g5u+?wT×i|$"?¯ù£Nâà?©d¥¾bs4?í·º–ê=?·øΣµ?˜¶yÆ÷h?¨rŽêscÀ?±¬ÀhüÀ?°ÔùNo€•?ìvš¼|?Ÿ4ù@zè?žlùü¦qS?–\÷r€?·áª`Í?˜o¾$Zz?ä^j9bTç?´¸µì ç?'÷´!È6A??Pwç˜*?Ö°JyåŽ?´j"-K½™AGN4FGL J2106.9+2455¿ëþíFûùÀ-Ýãø¶À:êﲪâ—À<3¯Rhƒ@À0"eÛ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@	Ýä$g?ïÿÿÊPË¿â=zŸXub¿ê•ñ¤ª[¿é¡­>¼ÿ$¿ïü¤–LÝÿ?¶Ýßnºó±AGNbcu3FGL J2106.1+2505MG3 J210642+2501?ïÖëwîà.?sÕÐÁ?8 ÍïÀ½Ç?8ÃÕ.dF?s7/±'e?s@Dݐ?ïáϊ¹¤?b<²â?iÓ¤t™?wbÀ-pë?†?—Nù}Ô?‹Ø!¸¹$?î¿ôC«Ê?'Tl+ï?€pDž;›é?{}H!"ó?ŸÉ¿+wÉ?˜š¶½%?ïZ'hj?8«ŒÈM?`q×À¿ ?EîϋôNç?šÆrÝƃØ?}ð[ç‰s?ï°u=ı ?'6#MÆ*?Bó÷Ú5?CùnÜU'{?'³)›üÁ?¿õkú0?îÃq0Ég?©â4øa#|?'wAMÒħ?–9އ°*?žV9]ôÆÊ?£çDË ¢®?íÝoo­©?–ž}øáû?lÐ~VHì?'X¾EÛ?ªÍÔãn5?"‹¼2Šg?í=àI<›"?ŸèB¢{P?s~!ÄüîÛ?cB8ûÇPª?´Ù™l?Ÿ¥Ù¼ööAGN4FGL J2325.9+6206c?ïþ4ê "h?ëê*«¥4ØÀ9¼iVïSÀ:øqž¨Í@5ü+46=@¡ÿ›¬?՞ë@]ñ«?ÁœßÉw?öæó^ÜÚ6@xýz>µr?ç}ÈMKŽ?îq!ôœu¿ìz_í{n¿å÷QÕR¿ïö¸ÞÙ>Ë¿ïürAeûÝAGNbcuNVSS J232543+6208290?åÁ€C¸‰?ÇRI/ì#L?¤ŽioV?¥?›3'•?ÑúŽ#ø5d?Æ+k_Šˆ?â¾7Yø2Æ?ÏzÏP)[?£1­WS³b?¨Ç	ßêÆ9?Ø[¡wš§?Í6EP0?ß@bÁK?±p:é2?µþºï¸[½?›é+åýn'?Û?ï$¡±&?¯ÊÊ'K?ãXÏ©Ø?­êÇÔRm¯?²f*"á?•®8´'É?Ôɛ9¬Éø?­(™œá²?á%ÃÆŠ?Ǟݚy?¾@8ÝÊ©?»"þC+<³?Ö$j@n7Ê?ŖED`_Å?Öº€O׿Ö?ÎÚ8¹7¢6?ºZr´ŸÑ¹?ÁÝõ&Á?áWq€%Þ?Ï»
¾ØÝ?ÒƬÞVT?«¿.'~f9?À؍Ľùd?¤ROxÑ1'?âf†¥rý?®)"ïYÁ?×â"9³U?´Ý—(Ü?¹¸º¤´³Y?©gvBÑ?àמ/s?¶Q#Ç&èMIXED

==> SOM_VIZIER/4FGL-DR2_prob_catalog_3classes_SMOTE <==
SIMPLE  =                    T / Standard FITS format                           BITPIX  =                    8 / Character data                                 NAXIS   =                    0 / No image, just extensions                      EXTEND  =                    T / There are standard extensions                  COMMENT Dummy header; see following table extension                             END                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                             XTENSION= 'BINTABLE'           / binary table extension                         BITPIX  =                    8 / 8-bit bytes                                    NAXIS   =                    2 / 2-dimensional table                            NAXIS1  =                  398 / width of table in bytes                        NAXIS2  =                 5788 / number of rows in table                        PCOUNT  =                    0 / size of special data area                      GCOUNT  =                    1 / one data group                                 TFIELDS =                   47 / number of columns                              EXTNAME = 'C:\Users\Matti\Downloads\aakash\Fermi-LAT\SOM\SMOTE\4FGL-DR2_prob...'TTYPE1  = 'Source_Name_4FGL'   / label for column 1                             TFORM1  = '18A     '           / format for column 1                            TTYPE2  = 'cos(GLON)'          / label for column 2                             TFORM2  = 'D       '           / format for column 2                            TTYPE3  = 'GLAT    '           / label for column 3                             TFORM3  = 'D       '           / format for column 3                            TTYPE4  = 'ln(Energy_Flux100)' / label for column 4                             TFORM4  = 'D       '           / format for column 4                            TTYPE5  = 'ln(Unc_Energy_Flux100)' / label for column 5                         TFORM5  = 'D       '           / format for column 5                            TTYPE6  = 'ln(Pivot_Energy)'   / label for column 6                             TFORM6  = 'D       '           / format for column 6                            TTYPE7  = 'LP_Index'           / label for column 7                             TFORM7  = 'D       '           / format for column 7                            TTYPE8  = 'Unc_LP_Index'       / label for column 8                             TFORM8  = 'D       '           / format for column 8                            TTYPE9  = 'LP_beta '           / label for column 9                             TFORM9  = 'D       '           / format for column 9                            TTYPE10 = 'LP_SigCurv'         / label for column 10                            TFORM10 = 'D       '           / format for column 10                           TTYPE11 = 'ln(Variability_Index)' / label for column 11                         TFORM11 = 'D       '           / format for column 11                           TTYPE12 = 'HR12    '           / label for column 12                            TFORM12 = 'D       '           / format for column 12                           TTYPE13 = 'HR23    '           / label for column 13                            TFORM13 = 'D       '           / format for column 13                           TTYPE14 = 'HR34    '           / label for column 14                            TFORM14 = 'D       '           / format for column 14                           TTYPE15 = 'HR45    '           / label for column 15                            TFORM15 = 'D       '           / format for column 15                           TTYPE16 = 'HR56    '           / label for column 16                            TFORM16 = 'D       '           / format for column 16                           TTYPE17 = 'HR67    '           / label for column 17                            TFORM17 = 'D       '           / format for column 17                           TTYPE18 = 'Category_4FGL'      / label for column 18                            TFORM18 = '5A      '           / format for column 18                           TTYPE19 = 'Class_4FGL'         / label for column 19                            TFORM19 = '5A      '           / format for column 19                           TTYPE20 = 'ASSOC_FGL'          / label for column 20                            TFORM20 = '18A     '           / format for column 20                           TTYPE21 = 'ASSOC1  '           / label for column 21                            TFORM21 = '28A     '           / format for column 21                           TTYPE22 = 'Flags_4FGL'         / label for column 22                            TFORM22 = 'I       '           / format for column 22                           TTYPE23 = 'AGN_BDT_S'          / label for column 23                            TFORM23 = 'D       '           / format for column 23                           TTYPE24 = 'AGN_BDT_STD_S'      / label for column 24                            TFORM24 = 'D       '           / format for column 24                           TTYPE25 = 'PSR_BDT_S'          / label for column 25                            TFORM25 = 'D       '           / format for column 25                           TTYPE26 = 'PSR_BDT_STD_S'      / label for column 26                            TFORM26 = 'D       '           / format for column 26                           TTYPE27 = 'OTHER_BDT_S'        / label for column 27                            TFORM27 = 'D       '           / format for column 27                           TTYPE28 = 'OTHER_BDT_STD_S'    / label for column 28                            TFORM28 = 'D       '           / format for column 28                           TTYPE29 = 'AGN_NN_S'           / label for column 29                            TFORM29 = 'D       '           / format for column 29                           TTYPE30 = 'AGN_NN_STD_S'       / label for column 30                            TFORM30 = 'D       '           / format for column 30                           TTYPE31 = 'PSR_NN_S'           / label for column 31                            TFORM31 = 'D       '           / format for column 31                           TTYPE32 = 'PSR_NN_STD_S'       / label for column 32                            TFORM32 = 'D       '           / format for column 32                           TTYPE33 = 'OTHER_NN_S'         / label for column 33                            TFORM33 = 'D       '           / format for column 33                           TTYPE34 = 'OTHER_NN_STD_S'     / label for column 34                            TFORM34 = 'D       '           / format for column 34                           TTYPE35 = 'AGN_RF_S'           / label for column 35                            TFORM35 = 'D       '           / format for column 35                           TTYPE36 = 'AGN_RF_STD_S'       / label for column 36                            TFORM36 = 'D       '           / format for column 36                           TTYPE37 = 'PSR_RF_S'           / label for column 37                            TFORM37 = 'D       '           / format for column 37                           TTYPE38 = 'PSR_RF_STD_S'       / label for column 38                            TFORM38 = 'D       '           / format for column 38                           TTYPE39 = 'OTHER_RF_S'         / label for column 39                            TFORM39 = 'D       '           / format for column 39                           TTYPE40 = 'OTHER_RF_STD_S'     / label for column 40                            TFORM40 = 'D       '           / format for column 40                           TTYPE41 = 'AGN_LR_S'           / label for column 41                            TFORM41 = 'D       '           / format for column 41                           TTYPE42 = 'AGN_LR_STD_S'       / label for column 42                            TFORM42 = 'D       '           / format for column 42                           TTYPE43 = 'PSR_LR_S'           / label for column 43                            TFORM43 = 'D       '           / format for column 43                           TTYPE44 = 'PSR_LR_STD_S'       / label for column 44                            TFORM44 = 'D       '           / format for column 44                           TTYPE45 = 'OTHER_LR_S'         / label for column 45                            TFORM45 = 'D       '           / format for column 45                           TTYPE46 = 'OTHER_LR_STD_S'     / label for column 46                            TFORM46 = 'D       '           / format for column 46                           TTYPE47 = 'Missing_Values_Flag' / label for column 47                           TFORM47 = 'I       '           / format for column 47                           DATE-HDU= '2022-01-29T22:26:19' / Date of HDU creation (UTC)                    STILVERS= '4.0-4   '           / Version of STIL software                       STILCLAS= 'uk.ac.starlink.fits.FitsTableWriter' / STIL Author class             END                                                                                                                                                             4FGL J0001.2+4741?ÙùË WìÚÀ,­º<§À;J,Rƒ[À<‡éÐ2@Qì̜{K@Þ¥šXÜ:?Ë·¢C6`¿Q¬gsùï?µz'Ÿ'h3@ù-@*¡¿ë8罓ô¿?讵¬ß¿á"c+YJ¿èÙE¡Iç*¿Ú!*•»¿Þ
\¿žúAGNbcuB3 2358+474?辶éV™?ÐîxÍ}®?Aëۍ'_?>즱Ѥ?"wˆ'3Š?XÕþ&?ï®Ãû7å?‹'²ƒã1?/·;ÓëŽE?TĊÃü^}?ƒÐ$LâXM?‰Õ¥ývïÙ?îP"ILŒ?'¬†õ'Ï?sa±}ðP?méCÆtO?¨'©[Ê+?†.-oz?«'mF?sùÌàq5?A11wŒ›O?74LÕÕ?ŒÄÂëäÊ?t–kk4FGL J0001.2-0747?ÞÕGqÐõÀPӅH©¼ýÀ9j8³¥´ZÀ<‡þ[@ŠÝÓÛ3î@"<½öp4?°Fc熝?¨ø\óvè?úƙ¬äÐ@ý"õ[?ïïXÌý¿á®?Ffí¿ã¤ÊOD
ò¿Úþ-b8Ú<¿èa~J2Կވ–<"AGNbll3FGL J0001.2-0748PMN J0001-0746?ïÕ܁JÛE?oE£7}¬Y?<FQà3I?4ñÞX¤º?sPZõtZ?n6>'ªB¤?ï½dïûo?…XÅ•Ë?:–dÙì#?R'£ì¿º?¤!´Öå?"ïLÜR?ï8ÄÀH!'?|$eºz£¶?eo¤Ò=!?R]¶`L½I?–9"¢a†?yõm7åó'?ï]Äì"?v=˜Œ£Bw?jwÁ»¹ï.?VÚ8‡¹n©?'ÏE/ƒ?sÝ\‡óy´4FGL J0001.5+2113?åyèÂÍÀDužèóÀ8^Äþ¢2À;Þ¿Â"O@O
"M@bœº¶IÔ?¡î[3?ÄRÆ6ɾ@L¦CÌ«@k˛ŸXJ¿Ï® yÈ¿äeßBp<ÿ¿èÀFA,ðú¿ìoN6ĸ+¿ïÿûÎBÓ?lÏÉëN¡AGNfsrq3FGL J0001.4+2120TXS 2358+209?ïȽy¾ˆ§?}‹ÖԂ:Y?uPyºñ?z*î–?YC%šŠ7K?`,"¹/R?ï™
c©8?ü.hÀ•.?Pî"äÂ^?w46ŒQ\?‡ºIk9Ê?Šã‰êÚPÆ?í#ðH5hÉ?¦†VQwD?¡$")wh?–h¥p¬‹?¬œwSü?¢ö•XÇ
?ïõîtØö;?KŒ/å}ã¸?2هO]iW?/óð•Ç—L?NÙhôxa¥?GÃåá¯<^4FGL J0001.6-4156?Ö$L^!†ÀRÓÃa@À:DOÀ1³×À<]yÞon@ —ÀÍe#?ú®oês¦Á?»xö"¼C?±ÛsÖôï?÷®·`,'@A=©-á:?í½¥|üªá¿ä«Kb©îQ¿ÑIò&ùi
¿ÑíñÀL5ä¿Ü}#Â'w¿Ïb9°ûµîAGNbcu3FGL J0002.2-41522MASS J00013275-4155252?ï"jˆÌùS?"ýÆ
nŽ?IA£>K†«??­®c3?QC˜Üòç?"Wò"!t"?œmbœ?ˆS…ïEåâ?9uæ²uÖÛ?Mw~îa?‡È©¯ª9?‡Ž|šÈ?´?î0Â1ÈÕá?'½'îà?qŒe¯'o?bëžV–Ä?ªÂP/¼±¯?Dw[¯Âf?î—
‡ŽT?…ÿ‡{=Ž?Y
ÛÕ6d'?FAG=çn?¥Æ¸¯]g¦?…É$¶¢Tü4FGL J0002.1-6728¿ãm5/EÀH{Râûã;À:'J7[·À<™øn;Fþ@ m#"'ÿ#?úؒ2>?Â	ˆ–.?Äõ¤îŒ@\	›Š4¢@Ï$'ҁî¿îèÌ!¬"2?Ï ¤Ð¯Z¿ÕºÀ°´¾¿ÔšÀ[¥B¿ÜÄ°ž˜Ý¿å«`"gAGNbcu3FGL J0002.0-6722SUMSS J000215-672653?ï¥SâԂ?wÔ1¤Ê²˜?aªíïÒp?ZV
Éhå?'@Lã"z?t|MÄê?ïThXja?"ǘ4—Á?Iš,̱ü?Z&òu_Úû?"¦Ž'à?"+qx4a²?î/x¨w>?Žxß·£åP?x¥Ìþ¥þ?h[¿:²¶Š?©óŲø·h?‹½ÀyF*?îVÜt"×+?‡CUB4Ó[?p<¹ñÉe?_õhK5Å?¨Š¡x'T$?†C=Ý$œp4FGL J0002.3-0815?Þ:Æ$'§ÀPöK	éÎÀ;\tì;'À<¥S"'Û@ 'ev§Q=?þÚ ø2¬?Ñçq"Á?Ã7S=êœA?óM¹Nè›@ŽM¡sÙ¿ïÿú Âî'?ïþ–ÞÔ6N¿ÝüK€ª¿Úmïÿ
z<?ïú;/€÷AGNbcuWISEA J000236.06-081532.4?ïëÛZ¥n'?]ÊSe&_?E¼8aÚIä?E Ö'f?]k."6Ž3?WÞ´&fç?ïw*=¬Ú?'ípòÄM?Rî`ˌ?cqí#W?ó­2È°?ó,¿•VÄ?íÍP³GQ›?'jÚ~?‰r³l*Ræ?¾þA©ž¹?¬ÎGð€Q ?¹L@R?î{#Úm?'r%ù:þ)?o†ézŠ®??f¶4^çOÁ?¦UU.°"?'e¿?0r4FGL J0002.4-5156?ìéSЮûùÀOÄþ'Q~xÀ;Á!\qÀ=dmgâg@ ÖKã*\?õ˜/6Np¦?áióïP…T?ä†Íyšö'?ÿuäô
ÿ8@/tæ±ÐG?êK7 ¦ê¿íƒgþìÛ¿èšð{þ~ ?ތ¦ æ{¿áL#ßÙ¿ïüò™åï´AGNbcuWISE J000229.20-515227.4?‹Àª?¢«ö"·y?YÀ쥶ó}?YtBYºœí?‡†õÈX÷(?¢•ë#K®E?s[c<?"ãôÆÀ^?O® Üå7'?h¿¶êÐj?‹YXÝ-?'ã‰s›ú?ìïðnxê?¡Yû3¹ã]?ƒ£P5tE°?y×h¦ÕƟ?¶¾uݯý? ÜÐD3=È?ï0^Î_'£?‹Ôcóµ²Ü?Iõ¸7ªH?RMyH7u¤?™$xrP{‰?‹¸ÉM´+4FGL J0003.1-5248?¾3M8±¼ÀOdüó0À:R"O…yQÀ<x|àü.º@ xŽÎ9‰d?üöYSXm?½°''¾?¬îþ%	yÑ?ó_6Ç<j?úжç2T¿éß5…
Ó¿ ©e>ž g¿áìáàZHK¿ÛY¶T»C¿ÑFÆbûLè¿äXY]ig£AGNbcu3FGL J0003.2-5246RBS 0006?ïI$l?'L,NQ²?SHÛ¦ì?Göy‰"Ê?œBQŠc#æ?õ	Î}
?ïQÛÏ!?–…Ô¡¦À"?ZŠv&▖?k¥v7&Ñ?"Þ»nR¥?"c
2Q]?í®ùpžs¾?'ÏÛ=?zwN¿‡' ?iÒ`ÞÝ?°à¿éá?'"2µˆ<?ìïWûÐa?˜Ê8\‡ÍL?€Õ;Š·dó?rl¢níýá?¶j˜¶¢Y?—ø"ýùû¿4FGL J0003.2+2207¿«mä›0Ù£ÀC°½ãû½{À;0')ˆ†À<w2>@­o@iBªI•?è¢Ç
,¸?árh!ýU×?ïýt³è@1¬šþ¨?úMEââ¿ä;ËB^n¿í5K Â€¿èuˆb—7?Ð;œ£º.å¿ïfKÄ#°ß¿ïþ'"oAGNbll2MASX J00032450+2204559?íÚXÔ¦sU?°º"@?ƒÏâw
?'žŒyÇ?­f¬/ ,ý?¯î÷ÄA?ë.ÿÙ¬õB?ÃÏ΋ ¨?¦Ö]ªÏFö?¹)[Úá&?»Ò]0²x?¹ïÿ}/a?êå秾?¥V1ñ1G?¥Dýæ"î?'®ú3=Èq?À¯e!êhN?¡ÓœË>'ß?ãW£m8±þ?ÅSÀ»ç˜?‹€ªTL±Q?œØh¶/ô?Øt³Òì6y?ÅÁ
ò€aZ4FGL J0003.3-1928¿æؾ&Z¡{ÀS%.ßç[ÄÀ:‰HºƒôíÀ<w˜¢ù"¬@qŒž3‡@w°év?À½mÈ°?ϊ' U`@
D žq@œåGB	?ï¬ýw޿δ]?KDw¿â‡ôiÉÈ¿ä`‹[uN¿ë°SO2m;¿ïÿùJYQAGNbcuPKS 0000-197?ï5¹×Ö¼f?ÚƒŠ¤ù÷?'½¯Y¾?Mˆ¦Õ¹?Hf-{êã?ƒðã†pg?ï}P/'œ?'"pr‹ÌÎ?RîY5òt?aR؇Xåø?Ž[öPr=+?ô<?L}O?ìECæ7ƒ?£\9ԝû!?¬t¾îaš?›YUŒH÷?¯:Ó;†(?"YŠ½ÉX?ï"Kð?áµJ@øc?gµ¤d'þ?XŒªS	"À?šF')ýŸî?}ö‹·J[æ4FGL J0003.3-5905?ïåòhâ+ÀL{¢£Y6À;Cü¯¨À<¼…Ñe¸Á@Ê\ñ*$@L€S?Á\¶î¿¿§~Š°¯?åýºËø<?øŸ5dæ´?ïíŠè%èMþraF¿åÉ3¿Â¿à8G¤Ú?|¿êwMt'I¿ïé\ AGNbcuPMN J0003-5905?ï°ª"€:?€"m²Ä¤®?P:Õ°os
?E¼v›©Í£?Î%%H?€*m̓?ïW%·†?˜íÔWg{?cV~"«­?kÒL	ú?™ªY<È>?—Z@Ì·(â?îƒì|"?Ë~îØ<Z?ƒ
£Ô
?x…¸t8á‰?ª9OqR?‹õ9jgeH?î	·,W¿?'©|ÌÔí?"¹Žs¡ì1?'™š>3܈?¥‡Æ¾?Xö/cÓ4FGL J0003.9-1149¿ï,Ä­»³ÀQÄÎp:ûÀ:ՇΕú©À<¦[·¶»@³9Õs?þéÀùYó'?ÄNmRé²?Ñ[!¤?ã@
¾á77¥?÷çÔåõé?êªI¥Ò?ïЊA7õ¿Øarv?!~¿ãMDVq%Ý¿ãªèvv~â¿ïÿò"²¢AGNbll3FGL J0003.8-1151PMN J0004-1148?î,
rŠm?¢BôlÈøÍ?œ¨9èE?˜Ì'ÃÞ=?Ö§Õc1?"RÙ}Ûގ?ê5<ds€G?ÇÃ[ç?²û²É,"I?½±¿\;Æ%?»Zj7i~?¾¥PÂb£§?êó©Åho?¨‡À³?µ=¸2Zñ?¢מÜ>?º:ª'¢a'?šI‡Ø£sŽ?å?±žˆã!þ"?¿PÒ«žÙ?­;¢˜7ë,?ËçN1—?­$ƒƒMª4FGL J0004.0+0840¿ï€ž¤#ÀJ2ìž#lÀ:ߍè‹o4À<&Žà4@aÖQZæ€?ú­Yº†y+?Òè‹o4kB?Þ×e,)ª@,œü$©-@oô0¿äõj¿'{¿ë÷]>Êk?«§½ý.È¿Ùý¥ýÖ.¿í¥è\uKÜ¿ä
NÒËêOAGNbll3FGL J0004.2+0843SDSS J000359.23+084138.1?íp|7Âß?¦VR1?–¿ñ+Šà?'Ú"Ò±áj?­˜CøBŒŒ?¢Ì.§ë»G?í>Aܺž%?´‹½šûè?‰¯¿:tFX?™J¨-ü?²×ù2܆?±¯/˜²'T?êQòz>?n?¦XoD6?®A}*!+?—jŒȞA?¾mKoxóý?¡µõ;e?éYÚqÄã?¨\ }ÎR?‰,Îäû¾í?&[½ÜþZ?É»§é0…?§ÚØGöä4FGL J0004.3+4614?ÆÏkì`LÀ/µ¶¡è´À:A´¶U'À<	*K-%@Hó{bKú@7<'W…ù?ÄRéF€?±:Ë^¸?ìt1ËT&É@m­3Tk<?é"€­ºc?Ò,&äñ0Ú¿æÓu}°"î¿æ6J²È¿ïÿÿ²}@¿ë
CQƜAGNfsrqMG4 J000421+4615?ïÝ7KéSÖ?f  7¨'*?MI'›ÀÏ??E9¨‹Ž×x?kvSo»ö?c{BoÐÊ°?ïÇ¡4?'~ÿsûOò?4p¦3œ??LûOú›?{.kNBÂ2?\¶!ÑÜ?î-·Ñ 5ß?"éR΃Ai?†L:ùNn?~(êÊk4?§'t'·Ž{?'C1Åu— ?ï`"[_{?uƒ¸8zã?o%\!Þ,P?\—]ymç?XK:?rŒ#±oä4FGL J0004.4-4737¿ís?oNÀPâk΅3±À9酿ÈŒÀ<ê$Ìh@G:ï•#¾@o-d½û?´Á«†?·»Il°'@-  ôØ@½Î°|µ¿Öš¢bë݉¿äà}ƒ¹^¿æwž™¿ã%ªê#õ©¿éˆÒ!Š_¿ïÿàU?ÍuAGNfsrq3FGL J0004.7-4740PKS 0002-478?ïÑi'°"?¢¡á²ü?6xänK‰l?)@#=ɕ¨?uã°`Ù:?¢àºµ?ïÚÞÇÜ^?x~˜wE%ƒ?»o'`Y6?2F"þ¼Áˆ?r_tO˜?wæ³U`(?ïNü³%?y£¢.»­?iP–'8ó?bÞZuõß5?"'¤´6?vi¹RlÞ?ïî`±Ï>?N³Ú—Ny"?0ŽY4w¼?"ç_QòÆ?_.[Tdø?M
8ʈà74FGL J0005.9+3824?﵆`ƃ À7¸dàÀ9œSÆP±ÉÀ<"Çȁ@p!G£X@j˜û(¸?¶Ã0òZ¦?ÈNÇ"é¹í@ô±î$5i@
LPóãg¿Ë&'¢È¿ânyZ^ñ'¿ê
ªB^Ia¿ëD§>ȽŸ¿êg <¶j¿ïÿüÉï£AGNfsrq3FGL J0006.4+3825S4 0003+38?ïåp'À'Î?g®ðÏu.N?^š %:±þ?\Ût-d8'?V"¼Y¿³Ð?Xû²-wh?îêÐ"p? ©+…ñ?tÅqî?R}?ƒ1©[x\?~©"Ýi?šqŽ$.?î]Qöˆ?•›¼ÀX~?ŠY^ýw7¹?'!8ö?£"ˆ×ª?ç÷ù†­?î¦éý'AP?"…áA¢)?ŽØ`«›8ü?vùÎäË
%?›¶ùê9{?³¼®‹F"4FGL J0006.3-0620?êe¢@ÝîÀP¨òù‡@À;/#Dže/À<­\Ï
ï­@·-¶œ‰¹@ØTÛ#§¥?Í"ÆÔeH?ųNáåbÆ?õOl@!ð!慿ç0Ýî]@M¿·?ï.K—Ù¿ä'§
öbȿݶßz¤`ó¿è:Ë­èÛ÷¿É~-W|AGNbllPKS 0003-066?ïµa¤§ÈË?v¸Ü
,Ôò?P²©ä'^»?Hį؅î?€'A™ˆáQ?u]ºïŠìü?ï¬_£áŽo?†BüH3Í?5¬*‡©?H¼¥F€º?":·£?…«ÜïK3%?î×.—.
?†,sŽžn?l
'^ý¡7?a2ï³%÷? Ìng/T3?ƒ÷'<¨|?ïr$´H‡?tÞþ"6€?Pî ê!G?AÔ.]«!ñ?¹Ê"íÌù?tÍ'!3ƒ§4FGL J0006.4+0135?ïôEÁ͌³ÀM¦&þq‹À;'Æf>À<¨Ð©*0@t×#x€?ûÚЛŽf`?ÕaÂÍÅp?ԍŸ½~ü?ü
9‰Ž‰›?ý[ÛU{²~?é&>ÚH¶?Ž"Ñ,û-*¿Õ¹¼å#/Û¿ÝOõ`¿³_¿å¶³ «Ü'¿ïëñUBQ´AGNbll3FGL J0006.2+0135NVSS J000626+013611?ïx7Mu?ŽRuÕsý?[}vF H?Sm*…à´?Žm]òÞÞ?ìZ 8'H?ï¯kùÞ?š´°}ìž?gh•ç?q·Ãñ5Iˆ?šÝÞ\ñš?˜8ªäÙU?ìùÖ÷¥ù?šX]rk+?"E|Á£Ù?ƒÄ©'ÿ?³äh*g<?–
+õ!?ì5¨mr
?˜ ™¥È›?ˆ;0sR$À?z¬ûîp--?»KVˆª*û?˜6ZZ—4FGL J0007.7+4008?å]×Hs-ÁÀ5ùÙUmÀ:Ë
Tí˜À<fߥ¥@"Dˆ›¡?ÿ¿Å}M3?Ãß4®]uý?ÆøĤ•@á*¢jùs@	ýÛV}e1?ï6è)I¥e¿Ý'‡"-D¿ãœzõi¤	¿ØëÚcä+
¿êWAï8²¿æÞ+	Ë[AGNbcu3FGL J0007.9+4006NVSS J000741+400830?ï'sŎM"?>JÔR	?p G֍þ?kÁ셶dt?ƒ[>xWÝ?z40Àv<?ïB¨?¹=ÏAÅ?PEÙi,"û?d¹ñ$A?´tM0MZ?‹+µCZI$?îQEw°ò?" qó-öË?†nùY#,?'ÜÃv/`?¥OêF^¨? q-Ô?îºí­œc?؇O\?z·ŸÞ©?hH8õ‡GV?Ÿå‹")?{ò7‹jVa4FGL J0008.0+4711¿ãQgÜ]8•À..¥.ùÀ8¹¢‰à¿À;§=áâއ@ÞTû½?þÛ«©gm?¦%"¤DÃS?´A﹋Ò\@®jv–_R?ýÉ
mAL¿ßÚ£}ɿך/ ~û‰¿àŒ
ÑyÛ¿ÛsËßgD¿ãéoÐrs»¿æ3R3ÐèAGNbll3FGL J0008.0+4713MG4 J000800+4712?çْx‹C?¼Y"þV§?'ÙǕøwX?ú?^_þï?Î>}+ã?»Z£$¬ z?èoï ô?É9#ÇÂ)}?Â$Š¼—·?Åó—[rþ×?»3k	Èì'?¶ÝrÁ€?äôEX	Õ?±B›º4¥?¯)¯§:!‰?™_"gö;b?Ò2?[œ$?®>"ŒÏiÖ?âüGzTß.?±"Vř?ºùU&´?¢q5wk°?Ӈ÷ö?² 8qu84FGL J0008.0-3937¿ïžÈ6SèÏÀR¥UGZ1¥À:½ÆßîÀ<xLuúX @Ñ"³U@+ã	O4?ͺš›!Y?Ú
‹t<è¿@»íx:¤@7Š:?îãË\4¿á롃rç¿éï¦`ÒRÉ¿ë:Ÿc2)¿î_ÌqæÍ¿ïý
':"AGNbcuPMN J0008-3945?î(¤²1Ï?¡%jãyk3?'YaÌʂ?@«vu©?¥âÉö}í?œ†¬E¬Ï?ìFSþ…>?¾¸ìa†êd?¥wHíúøù?²(ž«Í??³»˜Y"?²Qkã§;?êh%_μ‡?§V9î…?¬Ì܅'D[?•$؀	‡ž?¾Xf¾Èùš?¡ÈIïÛ¢y?çu«û_?¬Á¹±=¥Í?´…ׁaTœ? U®Šisx?Çèٓh6?«Ð=ûcµ4FGL J0008.4-2339?ïÿÿàSÀSì6ŸÏ=ÀÀ:Èeü´%À<{¼Ñ­^@!"þäÌó¹?õ•ôäC?Ñm>Fâ"?ÑͅC÷%¼@xCx%@påÆBð¿ïîÎô©‹?ïùÑb]Ã*¿ÆJ>¨nڿǯ³ ÿ)¿¢/¿œsÏ¿éÍáõ¨äAGNbll3FGL J0008.6-2340RBS 0016?ïÌöÔ
OŽ?vô‡ÇèK?Dá½w/þÎ?Eïq«°ëü?vè^Jr9´?tú>	MŠ?ïµuþ"?"sµÔ…<»?7_Kã@¢"?MÐ䥢ˆÙ?ç† ™þ?ƒ¢g)ÛƵ?ìùþ–%c?œÄAÇ~÷½?‰C<ŒÄ?…ª~B£Vó?µ—£ÍÃL?š¯X6ÿ}Ñ?î¼É;'M¿?]òÁžý?G[Jðu–î?A{/c8["?£Õÿ)M«?'íD¥ó4FGL J0008.4+1455?ã¤Rò/ ÄÀGVžšÀ:J‹¤äPwÀ<fjbti^@¡Úõr?ÿÈ+}\L?ÃÖÅIُ?Ä|í'hr°@_&¼,k™@Ðÿ¿EÑ?ïñÁä;~[?ÀV5VNb¿ÛAÅݚOw¿àðž'ú¿ât"Ì¿ïÿÿ)@k*AGNbcu3FGL J0008.3+1456NVSS J000825+145635?ïbøû¶ïœ?ƒÝKɶ?rH½R'5?jqLãv[?ŽbiCÐn?€·pt†
?î#¤æ'ȵ?®†ò·D¾?wé¾+=#G?€Â .Wù:?ªÈyÑkÐ:?­fÜc‰Ñ‡?í;@
üú?™mI»­?•ZRh^?TíDä¦?´#zµN‹$?•M°»â×?ëïÖèµq?•_7'Ü"?;%·…?"˜VkäQÅ?¹2QÁó1?''7ø+4FGL J0009.1+0628¿æ+xïÞÀKo$cŒ—SÀ9ö™"º]À<HßݵR@(É°7À·@*¢jùs?¶½'é("3?§_¾EdR?ñÇ=áâއ@Œ@ž'?鸞—@¿ÌGNž·Ì¿ãéˆà
ò1¿ß@?
Vñ¿á¨–¾•¿ßç¢ünÐîAGNbll3FGL J0009.1+0630TXS 0006+061?îáæSÐ@w?'Ã0À?c´
Ä?Ubdž? °Ÿ'*æÔ?'†/ø¿Èá?ïr¨ÑBC?KãQá;Ø?QèÖbT?aÔÞ%û¸?š'JQwË?:ß!X2?íxÜ´MO?—.,Db9{?ƒg8Í0Û?vÙDm-P?±Í$3Cïq?"õ¿zû"?îB›…',ê?‡_Ÿ_"­?~td ¼?hÜ;SÄô?¨»#Ùmû?…S!¬Yð"4FGL J0009.3+5030¿ïÊMùTŒ—À'›oâæê…À8mKrÅzÀ;•L''Ù@»-݈ܳ?þ\Ü_? Ï¯Ù¡ò?¯ãçñkg­@§óþiýË@˜p=Ö?µ,ü€kö¿Ý€Á›ì/>¿ày`^dL¿Üdµ÷ž1¯¿ãL
Ìsá¿á¡ê€¼ÓÛAGNbll3FGL J0009.3+5030NVSS J000922+503028?ïµq‹Ê?€ådUïòœ?3æù쮑…?.:{º ?'ëͨn?€¶w2ä/?ïÁñqü?…XiCÙi+?:-ݏBç'?RDEq+Å?}Ù)n
È?"iÝѲ?îæ*È,@?‹Éÿó•Œ?yºý¶Ÿ¢?s;ºÊÐg?œó8;P ?‡ó€‰DH?ïs'‰.…Œ?w¹L™à	Ž?Q*˜fXvú?@¾¹ªè?{%SÉÆÿ?w>Ȅi4FGL J0009.7-3217?é3ë¿×ÀSå¶ÃvöÀ;
Ë
Tí˜À<ÄFdh_e@I%Â1hX@¸¸]©ÿB?NjÑÅZÄ?Àq<XJï½?÷­_™Ã‹@л¸¨Rš¿ì)ˆ$&Oö?ïþ"4­†¶¿Þ5»8OÒ¦¿ç0ý~E€=¿Ùm"Ãqx¿ïÿ÷Âé±AGNrdg3FGL J0009.6-3211IC 1531?ïÝFÏkYh?}'Ã¸Ù'?E˜±ƒ4"¥?Zaé¾äŸå?mS3ُâ?zœ=bðø?ï³
lW¦	?ƒíy "Òz?9q#÷"¡?P‹Ã²T?'qÊ^yñ?ƒI˜ÈߘÉ?îWxåØۇ?Š»+d8µn?{,r¡™?qYˆÚú²Å?§$¬Ÿ?‡;03?ï—çB-	¸?rlzjõå ?Vðþ£¾?Mq×<¤Þ?‡61Té0‰?q«ˆïؘå4FGL J0009.8-4317?ßà‡ÉQ\ÀQñíåKIÀ:Ì{¥'Ì À<¿¹!]¹@¤ð'õJ@_¨†œg?¿ŠŠ2‰~?–ÃEÜÐrk?Ù|xl·c@¡d½Cî?ïý7˜ól¿ãGêüó¿àeê«%)¿ãŒÿÂÃ^¿ÊËîÖaöë¿ïünEWøåAGNbllSUMSS J000949-431654?ïÀóoÚÑ?v¶ŒYÂy?Fò‹ãk??>Š-‹&É?|¨̺ð?u´Šø"Â]?ツ–2ï•?ƒRoúH;I?+—æÛÓW??>^Æb«?áõ¯©šú?'ÝIK¯'¨?îoo¹ÂG•?%þ®«O?pˆˆM?b3¾6fç?§TrÛu˜?Žmg…"aò?謁ô¹¥ ?mB"Ǻ.J?@ã l¦%ú?5ÝÖ9•µ?"BÊÌ5 ?lÿ0o4FGL J0009.8+1340?â쀈óÑkÀGüU\Rç.À;W
F9 5À<Ÿ"Ì'úò@5 t-Þ?ÿ1-=¾§?ÝI–a€Îr?Ìô@ÚÖ?ñDœ¸2@ý³Š²K?ïâu@ýA¿ë¢&Á	õø¿â¦2ƒ
¿×Ï`ۍ
¿æÊf¿ïþ^	 '²AGNbcuRX J0009.9+1341?¹Õ§?'–+\h³?[ÊƁd}'?Z™ïïX?"axºo†a?Dm>xX@?ïÑÐJ?—`'gnMÒ?Z(¼_o³?k_X.\?œþÉ?–$Èä ã?íëvÿ0³?' Y'í|?|qÌ9&{¥?rkïZ¸Ì?­ºeHè%e?º©šÂc?í¾E_Y‰ƒ?"ÿصǪ¥?]vÜà˜M'?WsÙ΢{
?±—ù'±R±?"ï½€AŠÃ4FGL J0010.6+2043¿îæQ¶´ÀDk&¿‡jÀ:àÛŽ,~À<W÷7Ú@ïùR¼»]@þÜ~ñw§?Ê9R‡w'?µ|Û·Ì5?éðüVþ—@
ZɈ'?ïÌöˆ‡ù^¿à‰Éb4'¥¿æ8a¦
Ec¿äyïøK¿ïý÷è‰ø?ïå Jù"–AGNfsrqTXS 0007+205?ïåO|¦?rC îåÖ?.2°Ð›Y?&rÔ,­?hͽˆLß5?qûZË£]ø?ïK-…7»?"*1OÖJ°?P®Pö(?bWO­ˆ3T?•™"jI¨—?"Fãm¬?îÞtÞK­?".lãhž?rà¨i2ú?i¾¤UŠt?Ÿ¾ù:=Ž?á'Y²Ð?ïA——[‹p?ùÀƒìÏ?S}OEMu?CË°HΟY?–•8 9ÁË?G]|úå4FGL J0010.6-3025¿åba'àÀTÞ?»×²À:-úNwÀ<‹3b-Â@g@õ¼@$
COàé?·Œ~Óð'Š?»)Üâ‹S@R'IðäÚ@Éh>WÔ?é¡ªñA¿âLý|íç¿å9ΛÙæ¿ë÷…¿â¨°"rпïÿ÷fÔJpAGNfsrqPKS 0008-307?ïê ÏM¨?dIJ¯[q?(,|äŽ&?!ò‡ÄE?d\iiu?c禤¿y?ïÑÃ~y˜"?}úÀh¼à?%ï";
üå?Gf‹Ç̜Œ?vnÄ¡[–Â?{Åïéë"?ï&¿{†*
?'gƒ'ýü?iyÐb[{?aZË=œ"?—øւú3k?ëÃ!²?ïè,nO~?R,*†YÙe?1ÍcTjD?$± Tô»?e™åN·\	?QHΡE4FGL J0010.8-2154¿ê'ß9РÀSÙ¡ß¹8›À;3ö Û­:À<»:{&@jˆûf¾%@nLa…V?ÃÍzFÃý¿«H^éop?æGߒ¢."@ž¥]òú^?ï߂ˬç¿Þšù*3°¿æý¾Ý ¿äƒž?ò¿à¥R©®e¿ãûxFbºàAGNbcuPKS 0008-222?ï=·¹æÛ5?¢Q;a==?\ÑÖÆx´?cnÀ9Ðz?–{ëV½>?¡I²nØS?ïyOë.?—qYîm?Jcàp'EU?_5üŽf?ýÿ-ƒ?–hY'H?íÜ« ìps?öŽé0?|ãâ26Û°?g–ß3Ý<´?®˜Éªòg?9JÑt&?ïWŠÑã¾?{oeM­?R$®Ái?IèH0Ôlû?"ìd˜³q?zÔîM¨Y4FGL J0011.4-4110¿äDٍÇË©ÀRn!ÄuæÀ;D°P$ÜÀ<³@ý R@v^í T^@(z§f?ÐѦü-¸u?ÄCcW`€?ðö›r¸?ù©«?^dº?ç"0ý
'¿ç§0@9«ó¿éPÁ^.´s¿ä¾cþW3n¿ïý
ýn«.?äógkI$AGNbcuPMN J0011-4105?ï—!DA?…¤V¼Ã?a{¡®O?dgK²ÿ¹®?…ݏCYk5?ƒ•r°‡Ê?îŒ$Á°ë?«Wš|X?~=5⣳?½¶iøFÓ?£v
(®;_?¦Çì?ͳ?í¦Ú ŸŽ?"q
k‰9?Š6½ˆðå1?}ÃĂN,ë?¯®"Êåi?²ÜðZÄ?ít9ÿûß?˜Йҵ<?"pÞáE?ulÞì÷×D?±Ð.kKø^?–ÏÑþ±W 4FGL J0011.4+0057¿Ó?d©ÀN&¾œˆacÀ9ô–Å©ÂÝÀ<N­\Äüõ@L€oüè@IHÜä.?»ÞÿÝp^?¨:g³?êþ;¹ÿk@ö5¦Õí¿Ýù¥ÞÍ«¿å溌¤¿¿å×w¶á¿Û(RšǦ¿ëøV¿ïÿójÆGxAGNfsrq2FGL J0011.3+0054RX J0011.5+0058?ï»E(GùŽ?©~ñy€ö?R‡‰™ó"?|N]ÓØ?}»‰u†Së?¥ü§jR?ïܘ
UÉI?y†¬]C\?ÓiTÖ¶?>³º´ê˜K?q4­/È]?x¤0Å>'?ï0ÂD?'ùòu=à?u—-§÷c?t-ÿ(´?"ˆwÕ9•?z¬Ûäôë?ïÜÝ%G‡?\
ÆéÔ\N?6ROÐuw ?%ʁ¼=b?p,SpTå?[Ëp°íÓ4FGL J0011.8-3142¿ê¶—;ùÞÜÀTõƒ¥À;N²™DàÀ<ÓNáåbÆ@ 9ûIaó»?þ²ÜæöC¿?Ì]TS:?±]íÆídÈ?å>lý"O°@…'¤Ø'?Ú%â]ã°¿ëÚúWI'ñ¿â€
¡©2"¿ÔÞ¤»Œ¿Úyb&ñ†¿âd?Ÿþ¶AGNbcuSUMSS J001141-314220?ï± 2äni?y3˜hø[N?4J»õ•?'(¦%©Æ-?ƒnܼá?xÏÓaêo6?ïš{öÝÀl?Šífå
9•?>|Å>¿]'?Qî/N¢Û?ˆm™é"?‰çKp£§?îuþYÃêÐ?ŒU<7¹5?_Ô"x±«œ?K3‡Ó˜èò?§¡yOûű?‹ÔqìÉ]?ïfnô\ò;?yì‡Eý£ñ?2Mõ¦^\«?(Š:MŒ?'èéÈ??yãÁ"J¶Î4FGL J0012.0+7043?V+ìÔ@ 9(| À:Q/|À;Á2š†ÿc@
žÇ2@=v?ø="?¾Ñ8Ñ¦Ñ?Š›ÓRt¾?Ïý"ÀÁќ@tâÕø›?ï^0§g¸¿ç
µÂÅ¿ç
ˆ~¿¿ä'1}Ñg¿áEÅÜïüÆ$<kAGNbcu3FGL J0012.4+7040TXS 0008+704?î¹m¯…€?ŸMOÖÒ}?eŽa¿AY­?\:Y22_?£>ò3'h?žñZTª~9?æy‡6gïc?Æ_JèIfÉ?eÓ{a½Z?vJàûJҌ?ÒáJœl¦‡?ÆC˃º'?êÒËÔ5uç?©/*aób™?£M!"pa?{îRé	þ?º›Ýá]?§;ÚfM¸h?ì|ÍÍX>Õ?•Ù¹6;^?M¿¾é-N?i±_H¨ú?¹ïٝ`ã®?•.Ù@5OI4FGL J0013.1-3955?éf–õÀR»ê šª;À:¼b~À<vA
çI@½PdÇTé?þ¯¼†-¬?¸|)ò?½€{:ˆçñ@æ"FsØ@øv3xR¿îÄ"YFB?ÜR–»B᧿ཨ6ëN˜¿ßɯvz° ¿Ü¢‰'JG¢¿ïáGãÄ`AGNbll3FGL J0013.2-3954PKS 0010-401?ï£\Îá*?Ÿaßck[Ò?j±Îï'p?žÄuaVPì?€¢ßÔ?w‰YÖSÖ?ïiS
¯HÕ?˜—_2¦±E?Y¼§ègØ?rƒN<{×?'9Ô+gÇ?•Æ
åɀ?íÔêrtñ9?"ǪkIŠ?†xd	AV?{Á® Ƭ?­0º¿®œ? «¬'?îÙ+#G?"Ê…0°'?xvÈÏâò	?iuÎ‹–?ž¼éhZŸ?'ÎH'}×4FGL J0013.4+0950?妈vËR=ÀIóƒ@'À‡À:þ¨ø².À<Y·ø)qé@ (ÇÉ@ёW«¹?ÂGÞ;	@q¿±6"K~®‡?ççÛFSË@¼ë-`
'¿æt~7¸~¿éGúÀ{ٿ♅CÛ!¿Õ!â"o¿å®‹cuñ¿È2G%˜âAGNbcu1RXS J001328.4+094942?î
rDìÏ
?ªÿ²ÁOW?lÒXïÜk?†¹â'ÁÉ,?­‹¶"5H°?Â%뺜S?ïx¤'f*Ö?Œºw üL?CÆ'V6š°?RÔÁ¥~ì¾?M<˜ˆðg?‹pËuî?íÕdþ³?"—L<ce²?t΋ Œ¨?e
?TÍgê?°Û&¨^`?"…³ðŒ?îMöRTó?'!>–eÝ?\#v¾¡B?RÊ3~vb?ª?$ÊÂ?'D$ÍJæ4FGL J0013.6+4051¿áËsEòÓrÀ5svæj±À;ªáÀyØÀ<ž&~ïÊ@â¦J,@ÓjZç­#?Àz•ÈSÁ¿ª4
x¹z5?êE&z¾@@Û+'9֐¿ê ÛýÂ8¿Ð_f,"ÃI¿å¯wè]L¿âF(mÝS-¿ëyð¼–ä?ßú1Ÿ_VRAGNagn4C +40.01?îÌPž>Þ,?œ³'WŒ;#?x€\r_¿?tn>éúF$? *ê™CÑc?šÌî&n^?ïMœˆBRM?'ð(ˆþ¡Ø?NŽ¢IGDÝ?]q"³'0?•Wùåk|-?'A(«Ž"€?íˆú#?š'Óïl«?óTÛϒ?'/Pà3g?³ƒ¹ÄK½b?–ñ_æä?î²dàd?‹\;|K?mGmL5"¶?]¯×ƒTÅ­?£;*;?‹kR:¯4FGL J0013.6-0424?䝠ËxJ%ÀPcgM3HÀ:îÍ´SYCÀ<9òYNP@gzÃ?°D@Zþ¾·`T?Ԉx47¿±ÆÆ£gùŽ?ì´Ê(,o@r! 
Ò¿ì?"ÿ%åm¿ãm•ßû¨­¿êÑà2_¿ÛÄBÚÆ	º¿Ù›pß;9g¿ïÿÿÊPËAGNfsrqPKS 0011-046?ï<׸aÃ3?-ø—]°"?[ó"§U·Z?UŸÏ®Ž/p?–¥Ï©R>?œÎžò䁭?ï•7-]5q?Œ³™uSÒ??SžxêCc?R±Ú[~͏?‰·—´ëQy?‹[q«lò"?íL÷M'3?šJJ{žâ?'ùÚ½?p:Í}ìb?³Ÿ/Ýù&O?˜«íI×ðÑ?î9xˆx¿?'Å\—'Pu?P·t¹ì)?Fçæ92«1?«â»×μ?'ž¢sjïu4FGL J0013.9-1854?æ
ê‡PtjÀS…âlvKÀ:m» ÒÞ_À<…©²'b@K¶¤l[?ÿH‹¤äPw?¾`»ô?£Yÿ$ãº?æQSåZbL?÷¦è\JX¿¿êÝ´±M†¿Ã ÝE?û¿Ýc-˜pû¿ÝdŸý5ö1¿á—¬ÂkJ¿ÜFàd.RÏAGNbll3FGL J0013.9-1853RBS 0030?z€?€Òڒa?Nœ'
¾Õ?Bé´$®Ý?ŒÎ"
}?tmRâ\?ïQÄRûs?–8LRÒÍ?ZɃ¤g£M?g¤8•'^?"ç{Zd?"ïšJÿÈ?î"{j\ˆÉ?Œ"6eòy?yN>«—@Ë?g95 ?ª®"Ä‹T?ŠpˆÀCk?îJP"Ò?'{ðî?{Ýi€KÃ?mfI|ÂW?«¿­ÎÎ:k?ò©¸íš4FGL J0014.1+1910¿ãÙØ<ÜCÀEiÕ^kÆ"À:¤z
ˆ?À<ƒ€!ùO@ Y:ƒßs@<t$•?ÈùùUÁÓu?ÉD‹ÑYú@—Oµò–@
{I.óŸ¿Í-÷I£4¿ÜÔì@…4¿ãŒ'Á)i¿âñ¡§Úû¿íÇçÀn¹¿ïøðiŠAGNbll2FGL J0013.8+1907MG3 J001356+1910?ï[~°I9G?†¹ˆЪ?j~%öD+?b/ÇI?'@h2¢?"sŶÓ&?ïe#¯0?'4=¹¨?BÀÔ‡À?Sôñë•ØM?'Ç:æÉu¤?£Xorõ?îz°o2R?0C²|3?ˆï
Û)ei?€«Çú±¯º?¢2BBw?†K€æ灋?ï,¹ØL?}€´²el–?b{òV"G?N•"Öðƍ?˜F¶s;§?}45øZK4FGL J0014.1-5022¿ï¡rDQNãÀPlwÄ\»ÃÀ:"TýˆV{À<»à'ó@ŠÏ«úDT?ÿ{7(‹9…?Á
!«¡"?¡7öx±?àj|«LI…?ç¸øaœæ?ï(þûž¿éˆ—~6fÄ¿Ù#Ìhù¿¿áÝßÊÖS¿àg"Ý—ö+¿àp¯*$–¸AGNbll3FGL J0014.0-5025RBS 0032?ï"7Ÿ/x?'ß´öÉ?R±N·#?JÁ-wW®?ˆ›õrŽÊç?ø=¿JØ?íá8JÎÑ?µ¥ÖHÅ,\?öCiÝe?ž"€uú]?ªnêx¼ª?±\xª8ix?íÂ;ßIL?'üwÓÚ?~Jzíûõù?tñåæ:"A?°	yXåö>?ÓS¥þ»?æ3|@+jÝ?±'g«c°?¥Ù·ˆþÈ8?"øÆqÊk$?ÐÝЎ‰Q>?±™ö^	—4FGL J0014.2+0854?æ1'³ÆbóÀJm²•éâÀ:ÆL²`9üÀ<$ü.º'¯@p.#(ùô@á~4¹E?ÄBáÑ윿¢ÀÛkT?Û¬ƒå@ýTƒ™¿ï9¡v\Ô?ïùƒyœ¤¿åñ™ O–@¿ã.IW¿ïÿùŸé"Ú?ïÿ·ÀÌ
ŠAGNbllMS 0011.7+0837?קּͱ¦?€Š‹
"gk?lâ¥ÐÅ=¡?l±~©áœÞ?zË#°Äã?yô8H:i—?ïvȖHA?ŽËEgIÀH?LHø|?\¡LéÉW?Bï<wÌ?Œýjú´?ìb ¡ð{»?ŸÙõ_*?•4ÅÐ+?…¬ÇR.]?·Ž­ð
®?›ë'î¢Z?îïåÍb[?‡üDýSž?mdž>¯i?c8Hˆp ?žV²‹æñ<?†rAC§öÕ4FGL J0014.3-0500?àµRnÀP‹¬GG"À9þ!e«U"À;ó×Ûô‡ý@ÜÀ? ©Ù@Öæþ¸?¾á@øÔ2?¢hEÿ/Ý?äÓìŸ@ÀëNB-L?ë'm{-È¿ÚíÎm¿è¬l°{¿Ü;ŽK‡½Ï¿åÆ û;¿ðAGNbcu3FGL J0014.3-0455GALEXASC J001420.46-045929.1?ïÙÿ¢—~?s­'±–j?LZåŸû?Bz'Q	Ñ×?néÜo""@?ríN­CU?ï²æt(¸?"–.ìjM?5‹n¿ã?M@{·r¥'?'šŒoÒÝ?ƒÜ™=×
`?îVæ¯?–-;"'3?zXÞ`ˆë?pA`!¥?§F'SÑé?"9ž¹vË?îb"ß…Â?ˆìïÚ`š¯?qÚJx?^׸rÝ#?§›x¿•³ý?‡ôp"ÜC¨4FGL J0014.7+5801?ÐÃrc¯ZÀþ¡]³9À:ŒäxºüÁÀ<Uò#žjº@"R·Áø³[?øÙ<|ˆÛ?Åå¥vF®:?Ɖ·ú,×O@A&PÍ@‰¡a¿ïá@Âgîý?ïê'ñ¶'!¿Ó~°_-âç?­Ì8þ#[û¿ÔÜX[
葿ߥ83M4AGNbll3FGL J0014.7+58021RXS J001442.2+580201?çêötXR?À[ES''?rNDg,Œ?hú/ \?ÏÁ´:U?ÀE—Éê?ç,Ê:m´?ÉjÐhÙÕ´?SƒïÑ[õ‰?p
:¡|–ƒ?ђç›
È¡?ÉCpÐ6ÏW?éuàÜɸ?¬é;Üø?‰Yy`DÁ?tª‹Ö'Q?Ê`ë†ÔÕ?«½/Ø0?ílÈ=Ñ?•Xò´¬ì?{àà> Jo?j¬z÷cª?²áã»tÎ?•!jNð'=4FGL J0014.8+6118?åÁo'p@Á¿ôr6~ANÀ9u?èM[ÓÀ;×4ÊâçÁ@ Œ€¨ô?þjbßÉ(Ó?»M•ŸŽü?ÁëvÛÿo·@líԄQ3?ý
ÀN\¯¿ëgT7¹F¿¤^ÞMu¿ã¬Øpnýå¿Ùìý™É?¿ÞRe]Qꮿè
þEjÃAGNbcu3FGL J0014.6+61194C +60.01?èÊ¥²#—?µu"ä!?'?¸söêà?†Õ4Ȧž€?Ê­r(õH?´®kC<[·?ɉÎøVÑ6?ÂÏRy×ßÙ?™fâ7ÔÃA?¥([µ¾»Ô?èÒU0+¥™?ÂîÐ?o!Á?çQM0V?«µSÇ9>X? þPÐF?‰¢à^ºL‹?ϯ3òw
™?©V6{x')?á¥cýN˜ô?­Rcq·$?¹UQOEçÞ?£'©Y3?Ö_㱑T!?«]šMà=4FGL J0014.9+3212?ã"MäS@À>™»'ˆÛÀ9ض쐷sÀ<^xîÿ&¼@a]Uñy*@}_~ë˜j?¶'+èç	º?Áú
ø' Ï@5µœ.ŸP@¶`˜Ëþ?xî(g¿â–NöÞO¿é¦'™ð×n¿è€åM¸¿ï÷™)1Q²?ï]€C‡>MAGNbcu3C 6?ïæì×·ÖË?tIÒÓÁìB?T ,øí¨?oLö&	¾?^"°cY{b?e.žùN)?ïQ'¾í?ša›´'ìX?_ۗ"‡Ç?x!Šv'K?"Ò–
?–œ
^P$?ï3 ¬Ïš?yæ-ëé[Í?p"í±,?b$ÃlUç´?•vîùÁ¶v?vpSµ`²¬?ï¬U)ù
ï?màéqúï?p£yhó!œ?aî(3é?y1ñš…æÉ?dNü¬Çî–4FGL J0015.2+3537¿©£·­:g-À:­qGÏ¢À;x–z*h‰À<Í@N¤©@!8ÞZh×/?ÿKùƒ<Ú?į	Bsí㿤ä¯þœ
ù?âAªŸ¦N@¾ÌY	‡¿¦XåIpag?§‰\¾$›ô¿é§h5"¿ß¼MΕ¿Óz۞ ç׿Ö±MëE^AGNbllRX J0015.4+3536?îÉ¡è¬?™Š²œGò?WÃHQÃ?O<…¶]É<?¢§ÕQtd`?˜}¿í՛?ï9#ë?™¾‡«ì~?S`J(ƒGm?eZ—ƒ¾À?œÇ49N-?œ\ÓzY)M?íÅ'HÕWe?'oz‹+òZ?póùv'?[Ó²—,\Ë?°Ç†("ýf?'Ô¯uN;?íg?Y±êB?œÂèâThˆ?qaPH(²?h²4ëß(¬?³¯ð-î-?ZªcØž4FGL J0015.6+5551?´(¾ØEæÀ Õ}uv¥À:-ñŽM5=À<@â
K³]@!K'Z°Ð˜?þxòZ%?¹7ʜ›×Œ¿p÷B"ÓÈ?¶6)Ôº­@´€Ǒ?ïþrÎ\¿Ú),VJ¿âôÿý²H¿ÚP*¥Em¿Ûšëÿ!Û¿Ò£'™¾-AGNbll3FGL J0015.7+5552GB6 J0015+5551?궩ï48?·E'ÌNÃÍ?i®ƒÌ¬s_?a¨jH"ëy?ľ¡µ}T?·&¢ø.d?âTӪġ?Ä©a/ÝcW?Ws[å…a[?m¿»Yc´?ÚéâüÄñ^?Ě홰Ip?é>?¥sß9¾?o¯TòÔ?rè ¡z?ÉƯ¶˜Õ?¤•+ËßÍq?ëè1Û­@*?¹‡8F'0?‰×·îÒÓ!?u^p×ÐÖ?½ƒz$»¤D?ž±ê;Öo4FGL J0015.9+2440?î=Avö_ÀB¾µ²ÔÔÀ:Ñó¹À<~µI"ˆÁ@ã&T'Ÿ@ç!éB?¸@ï3t¿±¯Vš@ˆ†?ù'KiŠÞ@ºÄNÎð¿ã|VÝÝ@b¿èÄ(Lýà¿æ	¢–"¿Ú0±CŠÏ¿æÕu³
ƒè¿Í¦ÙÉ	žºAGNbllGB6 J0016+2440?ï«*"{?']ë=âh?dexwº?€'5ч?€ÃXY–?v®è‰Kž«?ï~J7N­8?ÛVXˆ?8Hz45…À?EBJÚ¤¸å?«.Z³2?‰ªsÎ~î?îÃð¹îµ§?ŠGÃ×ÕQ?lë©õÉ7Ó?XÈq"ÕÅ?¡ò9Á¸%?ˆÉ˜ÀŽ*?ïa)OV¥¿?zILž®1?`Þ^V<?PQ:¥ëâ?'غIj]Q?y¤Ájš$-4FGL J0016.2-0016¿î+Эï‰ÀNí$ò'Ð)À9oßÏpÀ<&4ú³å@­ã'K°@èƅŠîÜ?³{qæLOº?ǨƒÂAÙi@€8AíH@¢,**uõ?»\$š¿	¿åÿ$£Mw'¿èç6oþ•¿î´w JŽ¿àŠB
ÁŠ¿ï¼=Ó %¥AGNfsrq3FGL J0016.3-0013S3 0013-00?ïì5¹ÉÐ=?bÂW»·Iî?PIÃU¥ Ì?Q!³Ïðó?WJɹèÓ?X"4¬—Ÿ?ïŽi_ßX?"öñN‹Ê?Lž?4@L?e.Yý ?Š¥nXTåô?'ºÚšº}?íç9á}'?›ûtÀèŒ?'‹=*6$?‹Zvr÷B?¨IÌÍè?•0ˆÆäVs?ðÂ}?q™9æã$O?]ãk·Û ¶?UŸ‰Ú°?ƒ¡–'üè?nË"0ÉA¬4FGL J0016.5+1702¿Úª7h™hêÀFƒÑ¼râÀ:³dÀsøöÀ<j³fÊ9@0ù¼‡°@€ºˆ&«?Òç@ìY?Ó¡$'|œ@Ö_Æ	@[Õì¿æžï!‹k¿ä±^ýfr¦¿äì['û¿ëÇ4<G®ë¿ïÿ!Ÿ>õ?ï÷ZtÀœ=AGNfsrq3FGL J0016.5+1713GB6 J0015+1700?îp;ŒáˆY?£ÛäB-?^8ò7V±p?U™/<d°&?¨
 ,ÄØ?£"¤pød?î¡|ðµný?¢>Csß©ƒ?o¾*µ?¯Õ¹õ?£ìPáý¿Ì? V3`₳?ì»ìrÍÂ0?ŸBÖù'3'?–}¢‰õ?…"¢Z?´3ãJü?™1הR†ú?ï+UÏ?Šßµ0iµý?Zò)|…?Pî2Ò÷S?ërÅÜD9?ŠQœGl4FGL J0017.0-0649?ÞÅÄn.‡ÀQÙŽuyÀ:_ŠªŽÀ<`íjÒò@"†qsµ¯@9^Æ^ô'?·]HZŒ¾j?ŸÐ‡†5}?ægf
öÔ@
63ÍÔ?ïʇ½ùö&¿á#W¾,öÙ¿æ	8æ0¿àéT "¿ç6
]ÑíH¿ÛcS!DAAGNbcu3FGL J0017.2-0643PMN J0017-0650?ï¸~[¸©Î?sÚVÔ=?DÝ$âè?7V²"cû?€ŸÛ?‡kÓ?s7*» Ìà?ïÃð¾çÉ?… ''œ=?2ô]äï71?Q+ldþ¡?|Ø°Â='?€§I¤ÎÓ×?ï=C"7¦l?w;¬F¢½´?f;	ΰE?^Zç/gÀ?•,_5.Ú?umÈÅ1˜?÷®rf?h½°ËñK‰?ZVhIÖ?F÷€¶l?ƒÐµÚC$?f"³j?4FGL J0017.5-0514?èç˜8gGÀPª½Qï·À97@´%6À;ۀ
×Y@㵈b—@ÀÓ¢±p?­xm'—ýì?ºé'9Xç@	HdóŸŸ@ÁI©lJ?Ð]÷ÂnÏì¿äŠ&ßè³]¿è-©¼&Œ\¿ér*ŸÔy¿ár\=îx¿ïÿþó…õAGNFSRQ3FGL J0017.6-0512PMN J0017-0512?ïøÖ÷ñî—?FI:—z¹B?+U-nPÿ±?'³ªÇ^X?EÎÔܱ`Á?C7óà=ú'?ïш»ØÛ?|\cz†ÉÕ?(Y¯O'?Bs¨Åÿ'…?v{}˜êð?{^ܞ+0¶?ï枟td?…rºiŸÃ?s(ñks?i*‹.ølÐ?š8ïÑK¯`?'ÏX¬Â—?ïØ?¤Â?aX:Aû2¯?@8`ä",?5	R§1h?qïyl'Ö?`½†˜½h4FGL J0017.8+1455¿áZ3ŸŒÀG•{t¤ÓÀ:£ß\òI^À<‰f1A@s~"?jN@?L¤?Í_,
u?É$Bjۗ?ûqG6w@<¼K <v?ïý?ѧ¿ã/+f¶¿à("` Ò¿àøý!©H
¿æ6""Ý¿è­-]AGNbllGB6 J0017+1450?î=5¸•¤q? %k8ˆ¥?kÏÈø ?a°ì4ÙÌ?ªo³Š7+?Ÿ281åÂ?îíiË"?šGëYMÉ?U0'ú?]m[Ñû…? yï!ý:»?™¹"ɦI?í¦¬w‡ƒ¤?'%í¸=¿ã?ƒ·\iá?tÎ~=vF?°fÅX6À?	§Š›?î,=Ñiˆ?ƒç	xŒh?tú¼'lÐ?`ùîè$<â?ªŸ4 ¹å?ƒ
Ž¿ƒš,4FGL J0018.4+2946?ÌÍfŸ5(ÆÀ@F-¶°`À:[ŒõFhšÀ<RùôMDV@!JË
)úz?ù€ÝàñG?Á*Á_0g&?ºäeb…[?ü}w$#Ë·?ùjž"dÿ?ïx³ÀŒLª¿çHº•"<¿Äê0_ï(í¿ÐQõ–²Y¿álîu"Ó?°m®^kAGNbll3FGL J0018.4+2947RBS 0042?îx1ÈWY|?ž©Õg{œ?Z½Tv•p¡?R_7)F?§¦øÖÕ¼Á?žNvqà(?í×·Ò×6?©ïМ¯W…?€"·µK'«?ŠÁé÷,(Ü?®_Tå<ò¥?¦w`,añ`?íU›	ô'?™¼ "ÆÁú?}NÀ…±"n?hM¶…[¶Õ?µhgUC9?˜´îô9?æѶ¢f
?¨ó=;9?—÷¹?'~ªÑR™?Òu,cIâi?¨pb-לJ4FGL J0019.2-5640¿çÇ>­å«ìÀMòÜ­¡À:m'§7À<³[bý%Z@C+xÕ@_±%§Yv?º ZmO?¤-7#`_ð?éÔò5<!ï@O•¿ol¿ÂסçñÁ¿Ó§ŸÁ¦Óê¿åܟ]}ß¿ÜPLßÖë¿ç/§Ã(]¿ï¸uý³¦AGNbcu3FGL J0019.1-5645PMN J0019-5641?ïNŠ?‰Ž?³†ù•?[鈾˜±8?x¼.Öio%?"p"%C?±­MÂ0?ïßx4þµ¤?wƒ9€îhÉ?ÔÐõ?2Ð&›e>_?oÁ*šÂ³X?w
"4z÷Œ?ï@ëÚ°E?{Àd$Gc\?hJÄ{È??aC
= < ?"ö‰õ0ö°?x ¼À_q?ïñªÁ7?F"‡ºÆ95?#Sw'¿>ï?«a<Ýàr?ZAW…©Í?EæT[°ƒ4FGL J0019.3-8152¿í7™VÓ¡RÀA"¿]xÀ9µo`
+ÓÀ<IîsÂ@N1‰9úù@šbÞòi?³f"nd6¶?¥B<Ä	7?ò@‰ƒœ@½×¿â úa§°¿â%\°Úÿ¿á}Gô‹W·¿à\øɪÙ]¿à×~0‡‡¿èï;!>>)AGNbll3FGL J0018.9-8152PMN J0019-8152?6ŒôÕ?}ušæ¿?LïÏyŽ/t?@'W»¾¾?…Éue)çÎ?|J^‡vy›?ïr*b^F?'nÿ~BçÀ?@âœ¹—?R݉ì?''EÓNj—?é¸h:Cî?ïdæç"µ?…CÖ(¡Ë[?iêòzi?VƒÌü-£?œ¥à}Z?ƒ¤››0n?ïó…r¼?ƒ'Outv?l ڎcµ?WÞÍÏ£³?šýSÿÜ*?'‹5º]^&4FGL J0019.6+7327?Ô
zí±ô¯@%sõ/ÂekÀ8¬ÿ˜Ñó}À;cgž@–×í<X÷@ÛVà·e\?¬¶áAèœ{?²ûðü¬äO@Å6B²,8@DVÇ?ïÅÒr(;ˆ¿á
/þËLš¿é1rEî¿äõ¹?§4ã¿ï¨ÿ"_{f¿ïÙzé¯AGNfsrqS5 0016+73?ïӖîüŒ?sÔÏðÒ?S8­æä¢I?W›‰X›Š-?qf]7HØ?p!Fhuõ´?ï|{À×ÈÊ?ž"ì'Òýç?^sç‹{?‹Ã:BFd?»Ûé?–ËwgRm?톫³Ákð?›¨ûý?—;ÝJ=eÎ?Œdè"ä%l?«÷Vʎ?"úݕRí˜?ïr,ïãÏ?|(‹?.†?o¡!ºÇL?aãSé<Ù?‹Œ{±UHX?y‰c˜œÞ4FGL J0019.6+2022?ïbSßG›ÀDð\|ؙÀ:Z°,ƒÊÀ<|à"&þ@»½•LWò@è"ÿ‰;?¿Ì[㫌?¾[Ó µ'?ü§›4¤L{@*Ò2<h;?ïýròe㊿¥}¯-T¡î¿âë}'üf¿ãٔü{ç¿éì×.OŸ¿Ôܐ¤¨koAGNbll3FGL J0019.4+2021PKS 0017+200?m6?ªÚÙ»?ePÂ4ø¼Œ?huÓÑ}\L?‰éæ°¦ƒA?}{ÃãeW?ï
E™ˆê¥?"N¯{Rñ?[ûZ¢"–D?d&娌é?œ——$Àù?'óßÙBhG?î-ÈLV?'1Ÿ£'.?'_Ãc'?wa}ϙ
?©›‹´‰Å"?TÛÊqü"?Tl«º?ƒNç\"3?ˆÓ…'Ùn?qÁ<˜±W7? iQԎ ?€{6I=ýå4FGL J0020.3+6919?æRÄ}?hB@·¿ŽaÀ:>TÁù44À;£©8s@ºy³ +@ËYÝÁç–?̳*yÑ'O?ÈOÊB®Ñ9?ýóÂî?ãË(²H3˜?ï;ØÞ¨íJ¿ÈʺÂH¿ã¬Y?6vµ¿éZoíÎ¥¿ïÿú¡œGt?î  ¿'ȜAGNbcuTXS 0016+691?ä'°»Ð=?Ê>Li@y§?•¬ŸP(·?"Ú¸%îÊ?Ձ
"\û?ɧ°*tš?Ɂ>jG[?ÆÐ-¸–	=?ÃÐùÅfÑ?ÅA ö¬1?ä«qô&†?ǃVŒ»{{?ÝOø
Íl{?±6H°Ò?¸×˜å±J?™µ®ÿhh?Üz!¸ì'1?¯óI‰Ž?ÂF«U+?¥Ì‹õ—%\?̎1>Ä1p?²®v&ƒ?äJïïäY?³Ô›í™_4FGL J0021.0+0322?ÂÜɾ">«ÀMOÀãŠ~tÀ; a3÷~À<™A<á1ß@ »ÚҞóÌ?û6ìü=?ÐMØ%–¯?€Å'pÛ?õ<¸gºú<@éä.b?àI '–ó¢¿â!3E¨¿äp¹pÏuô¿Ïp-åk*¿Úaj~#Ž¿æ`–
õAGNbcu3FGL J0020.9+03232MASS J00205023+0323578?ï…+AÆ?½2ôp.®?C9bjƒ•{?6ûxåZ¸^?™"&C³?nìõzc{?ï¢d;"}s?‡¤z¤Úýó?8Õ>Ö3ç?J¡úý†[J?†¦riñÔ?†ÔÊî_@9?îMªà%žt?n`åðyP?eþð¾
/?R®)Ð#‡?©Åbûº7Í?ŽÀ4Xß¡´?î¥b"2¹¸?…N*4—
'?HÖ< >?>7Œ`d?¥F~Çä?…<ƒÄgK¢4FGL J0021.5-2552¿ÝÜ*¸»GêÀTÌǎŸj"À9¤GOIê/À<WëÃ¹ÿ@¯mŒöH@§¦tso?°/R¾hÛâ?§ùâ&Â?÷$êµë߸@#8Vˆ¢Ñ¿ÞgÃ}î˜O¿ÛyáBz£à¿á$ý°šg¿àl°Ý­ð"¿è=[‹`œ¿ÔÄh¥/úÅAGNbll3FGL J0021.6-2553CRATES J002132.55-255049.3?9´/?X»˜ÑK´?BWĈЏ??P£Ÿäª‡?…÷?©ë®?œYlKL?ï²<{ºf?
ŽÓݞ?5ܧA/ü°?S)ò®–þ?'Âçæk?<ÙUáµÉ?ï6¨þãƒ?€ðPçÙ]²?h1ÜvÔ§6?aÁÞ"7æd?–$¤­èú¶?~ý—K"4?ï°pt+­?jv"~¿×?R(¿]Ê?B¬Xé=?à?¶b	sè?gÒþág44FGL J0021.6-0855?&ó="£ÀQžc^J8À:÷ØcÙÄ,À<Ÿ#vý_@Ñ£žU@@DXÍ?Ô5lÉV÷?У–r¬?ûü'¶vI2@£&T'Ÿ?åð ±»ÏO¿áv+ÀÎð¿àvÔb˜P™¿æ.Å_ñ_¿ïÿþÐñ¿îkV斢AGNbllNVSS J002142-090044?`…Ú†?ƒ7Î`uŒ?jÝÑÁXË?g;"y¥J{?"eçj?€iÝmÓ6?ïÁŠÔ©@?›íïþ!Ý=?eA5e(e?pØî"<ö?š?­¾2ô?™¡kš®0w?ì\J‡Ì³h?Žg€‡?¢›J¨]¯?bk" V?³Ðmk¤Þ?"žB-@?íªÑ/uÁ?""æ~­h?€¼ÚáEØÆ?t¤E&œÝ?°'Û()<E?'»ÅàÔ©œ4FGL J0021.9-5140?ì³DSI±­ÀP5w ÈÍdÀ9¼•*™1À<i㤦©@ž4E,@m^•—?°F¸ Bj´?ƒ—»W¦Ò?Ñ}0'S×Ã@cː6Äb¿Ætž7ŽÇ¿äÑå©és¿ÞaOÛàf¿àLJžDy,¿Þá\ü°?M¿áñŸ,ݯAGNbll3FGL J0022.1-51411RXS J002159.2-514028?ïìÙ÷ç»?XKu¯e!E?0b±ö£[?+ô4LY˜?aêÏÉCáý?VÀø?ïÛòY5­i?xñÔ©þ?üx7–¬;?8¾JV&?q'á"Jñs?xHí¨Q–?ïMŠ¿ˆ¡?z'	OéË
?e©œÓŠQÈ?crÖRÇ?"™tt‹a›?w*'¡-d?ïáX¥?XžZ•:|?5–¯åšdõ?*W'ó|­=?l2Ñ]ͤ¿?W%a×î¾C4FGL J0022.0+0006?íÒ»ÀÀNí؃º4DÀ;/…(ÉÀ<~CvwU¢@#zISž?ù;ë2éaX?À2AƞàU¿®p——¶Àq?ï"{[>@×ä"Sçß¿ï&%z
?ïþC¢|l¿äVÇ¡Р¿ãȑ¿/«>¿à@óæJ?àâÙ,,¯AGNbllRX J0022.0+0006?ï¹mœœDz?"4zj5L£?7ñ‡d?2']¼èÛà?€ì€¸U˜?ƒëŽÙ$'˜?ïxIvïS?"Z<ö:®?P­-`]Y3?d-NZÄ?×ü˜'?'U"vcW?íÅÍ…	?–€Žñºg
?s?žýþR?g¶o6­?°é¨ò'?•È}¥‹ç#?êQò4'"´?´šÝ27|@?z§i7©7?|Ú÷z¹?Åâûå©é?´ð˜Vº4FGL J0022.1-1854?íuU¼
ü‡ÀS×õY³Ð}À9Ÿ‡mG+8À<æ¾æZ=@2ý2Ys?üI(gþ?´Y¢ž%•?ºë¬ "ÚÆ@¼uf´iÿ@#¤^º?î÷*¾ðk8¿Ýµ‡9᣿ևî@¿ØM´ÿ%ºz¿ç‹^Öw¿Òl"h	ԕAGNbll3FGL J0022.1-18551RXS J002209.2-185333?ïŠïðZ'?…^«Ÿ§†?ZxŸÛ€ò?WR+j?‰õ'ˆyv_?"»rºAÃ?ï?¥¿aÉ°?¡9Šòãî?blNœ?|j´VþŠ?•»‰ó:?žV'I»Ë=?í²t{•Hn?˜f«rTƒ?†ðÜ+ú˜?|Sì=E?¯;¬Ó?"¼_ðß ?íò°¡Ä'?–…ÐôÐúÐ?rðÆÅUf?cÛïæúºE?®væÂè?–l»	tÌ84FGL J0022.5+0608¿ïòü³‰ºÀLl
oTLÀ8Ÿ6}jŽêÀ;¢OYÚg@û£è§ô¦@|\qðÞ?¤ "ˆÞ`s?ªMúY
°@8ÑØ¥H@F_Á܃ϿÃGw£O¥Û¿Ý¸¼yBŒ¿ã7õfI
¿á0[è^"Ë¿ã–#£Â¿ê
©ÂÉnAGNbll3FGL J0022.5+0608PKS 0019+058?ïAï¯Ǜ?¢Çh_þÝÈ?E;ÿHÚ?NCœA«'?—*%uÒ?¢ƒÿXÅ?ï¸<@©[æ?"êˆîº‹?;"_:üÔ?TJÝ£åóÖ?ã:¯.¤?ƒ‰Qå7ð?îý9Y˜Ö?‰mnç?phÁ"^Â?gÚ3ŽñÉ?œEÈoõ4Ø?‡–™¤µÙ?ïR‰Yôqþ?€¦c_b;˜?S¼½6?B©Þݸʷ?"sî÷?€wQ+m\4FGL J0023.7-6820?ÝÈoY÷eÀHJ"‹ë[-À9òóú8?âÀ<' Í|@þ¥aùÅ@›2öÍ?µp(.mQ?µ áL
Ł?ø3)ø÷Î@Gs\/¿Ðj@ºˆ'¿ç3®eÙ¿éès€¿åÀþŠÓ¿ïÿþÐñ?äñ*å†×öAGNfsrq3FGL J0021.6-6835PKS 0021-686?ïëwZ1#Ã?‰m'ƒoÇ?_Åïß°UW?‰m­à}L?B–·|F?@¿ÚvFÝ?ïmœb~³"?•åuîS?SÈàËØA?n¾ÞžÉã?'å£l	€?"IŒÜÕ?ïRƒïŒŒÁ?u6akÞK|?hô?‡u£?W¬Äù	ju?'úÅÊ?s3´´72\?ïÚ¶Š@Õ¡?_™)&ñ?^Èfäň?R5áɜ\T?eåBM'úg?TÜÊ	·›4FGL J0023.7+4457¿u…º1ô'²À1¥3ã\[KÀ9¸AûMÀ<PZUÖ@ôrÏ«Nx@aE•6?²»®·Ë?²ƒ:\9â?þ/ˆØ6@\¼üË@?ïÅJŒì-¿ã¡Îò@û¿åÑ瞊D<¿æ‹¡>(¯¢¿é8}¿H€¿æ_AtyAGNfsrq3FGL J0023.5+4454B3 0020+446?ïî@ÿ?'ÿ‹Wíñ?G«xýŽ3?Tqþ'ÞÉ?{3Z­º¶?€±f´ùnº?ïуwÂ?~!tðµ¾"?20%7ƟÀ?Rȧ?i­?vB*4³?{ cÀpý:?ï,æÀì8?}¯œ{èS?k{í<Õ?^ž±ÆV'?—ŀ`•?zq)ßÇïL?ïÔÔE"ë?]d]#§Ã®?U‹·dàˆ?Bè£%v?p2s?YÛÐõ)º4FGL J0023.9+1603?ïGDRÀG%ƟŒ!âÀ:"¬ñe2ŠÀ<s
=Ö$@É­"£:­?ÿPœÐ…¿?ǸÖöœT	?ÀxxšE'?øZÁ¶%@S$彉Ž?ïâHZ⥿ã#˜ ö/G¿àsÉøÜö¿Õƒ
¼õ¿éÕ	ÖB—¿æòçHy–AGNbll87GB 002122.5+154553?ï €¡5œ?õ—yôëF?g½±oÛMñ?eþÜ)ˆ%?˜ø5«R¢¼?¼œÙG½f?îí´6XÌé?štîô'™l?`˜QŠü°?iíóÌ%Ô? #³Z®?™*éÏ©O?íÞ¡C#y?'?'WCïC?€QÈ,?tï|Jx›?®ñ§9Vd?Ž/~Üw?íiLe¬Rà?ŽlL)?ŠûŸ/xw?rîÈ2‹ï?±t^·yì?Œš
Õ?4FGL J0024.4+4647?Ôì%|*6ÏÀ/¥Þ7X[âÀ:þŠBäÀ<`;`(^Ä@½$Ö¤@Œ…=Â?Ã4øŤ"¿«Á}ä1m?æÀPQ_@	ïùÜOv¶¿àhˆ•â¿éiáyð‡¿ëEM|Š•¿ÊÐԙI聿ïÝˍ1¬J?î'¢ PØ`AGNbcuB3 0021+464?ïçÓÝ»'Ü?qÚܺ 2ú?=¦¨{tªD?<ϨÝwú0?dwM5i^?pZeL@?ï¤ØfèqT?˜3v¥¿?A|.v½?\??…¸þ'ü?
?'°¬3?ïÆLUžÔ?…ÞŸ)šý?jˆò'nï?bf.\fM?œšçŽ?"©¥×a$£?ï¿!.ƒ|P?m[Ái²Å?<æ—©^?4?~¡"ÇAÐ?lNÔ£é)4FGL J0024.7+0349¿ï75"ØR£ÀM0i@5z5À:ß[†8"ÅÀ<t{i,êD@Ç-õ±q@	þCg]Ý?ÈcŸŒ¢»?¼Ù©¿Š¯?òî^íÌ!@ê0ðã­d?Ä"SçÞ¡?ï–7D9ë´¿é yó$÷¿áß-WQ­¿æ¤õ8%á¿ïóÉü7ôcAGNfsrq3FGL J0024.4+0350GB6 J0024+0349?ïÒzmû×Ò?­˜]5Ò C?C¦ܙe?x}-JIп?tN ˜ƒ?ª‰krÑ+(?ïÖEþº5æ?}"FôC1?)à$	Š³Ï?FÛQ	LQ¼?t
ÿ'˜¸¥?|L͓ß
??îÌ}fzH?†#9^àœ?qÞ6÷'t°?dUòöÖõ? übÀá?"/Þ²LáŸ?ï×K'‡b?`^Ï]FÄ?7à"Á÷?/ôÿDMw?rÜ/)«ÎÇ?_|M'·›4FGL J0025.2-2231?ïåCûq>ËÀTŸ!BoçÀ;'›]:À<®ÑOŒÊ@u*ÑsP@#5ߵݝ?Âí'úÆ°(¿¢‹ìCíþ?ß¡J½éZ!@àë¡y6ù?ïÿÃF1=¿ásÁ}ä1m¿í§À8iÓÙ?°‡Ãs¢º¿ïÿØþ3w&?ïþ7ޓž®AGNfsrqPMN J0025-2228?ïâÝÌüìÜ?v·Ý<œ—'?B~Ý[9æÙ?FîoBß??h'{¬D¨™?u]òpÚ¹½?æ@åk?'O1ÒhEM?Lz.÷€^?d†q5?‹cƒ‹-Œ?'@"­ªP{?í"PÂG[?™ŠF¸Íƒ?qßZÇ ?v	ó‡÷aý?±±Ážl2?˜>Ϫ©?ï¹ZÞc½Õ?sLjó¾ÃŠ?YÕâ—Ç[Å?Wº{ZxÔ ?|Ý(/>ô?pÇöC\4FGL J0025.7-4801?ëґTH#ÀQ!©æî·À:aŠ ÒHÀ<"P/Ã<*@H¹»øê?ÿm…/J?ÍiKH'áñ?Ê3E½#Œw?ÿ±¦Ö˜þ@I";ø¿çqCĐ¿Âw&gÈþ¿äZ1®
j¿ßýäqÚ
¿ë	^î¢àj¿ïÿÀ¿ù)ÍAGNbcuSUMSS J002545-480356?ïà:ó…qƒ?†šßR1€Ë?F*\Žæ^?L–—¾5?j:…cjÁò?†
³fï?ïÛüçŠ?zS¥†‹D
?!qlLŽ<î?=îë8F³a?qv™ÉP?yN|)`"Å?î8L˜#ù?"	—Åõe?ˆˆTŒ‡UX?€ÉŠÆF¹Q?¦Y![«ë?èµbŠS<?ïê1ñ"?QÊ?‰ÌuM?#âf¬fŠ?"¸Y±N?d5ïè©û?Qž%ãôàw4FGL J0026.6-4600¿È&	Ê.6õÀQžÏ€Ü3rÀ:Îùn‡QÀ<µG› @헗‹ÍS?þë׉¿1?Á!q)búÌ?†óxæ¤Aò?É»g_4Ã×@üe+Rê?ï÷´×ãD¿ã§E‰w§¿Þ€§ZL|°¿×ÂC[õIC¿æ›ëþì.½?®¬ù$AGNbll3FGL J0026.7-46031RXS J002636.3-460101?ﮩÕq¨?¤Uªµx,?Eñ¶ÉuUó?bóin&o?'öœÞ@p?¢ò-×ÊÉó?Ö}?ˆ«ÓZ.Ü?9'\Ò)?QÒënþå?†ÿ€ë-?‡©ùËëÚ?î1¹UFî?bÇ$n?pósÄrôg?[£"‡!?ªÑeò2p?Œ@ëUùÛ?ïIRs¹G?x¹»Öõ¯?VMÎȺòš?B¬¢Ð3~À?•pÓ$ý'ß?xcy|ñ}H4FGL J0028.1+7505¿Ûø¹"ñké@(–G™ÅXÀ:Üéä4È_À<¶‡•@y56Ì?ü½3«(?ɯ_Éî?Û'‡W@
Ä_@wÏ@d
+' *¿åJ¬–Ì_À¿ê,9¿iaî¿­ª±ÄޖϿÚÛ5{Ù¿åøšá"¿ïÿGuܦAGNbcu3FGL J0028.6+7507GB6 J0028+7506?ëBLiÀÌø?²Ú®BuüÞ?«ÝU‡½ÍN?£xRª€³?·þñî±'?¯
W¡þ¿ž?èñf=?ÃxœÊ¶j?¥~}ÕE?¥»ß»¾ø¡?Æúûõêñ»?Áð¿°§?è°à¾iä?«ÏLzˆ$?¹óF´Yo?¥)S¬þ?ÀBÙ¬C¹?žÁŸ·E(2?éz/XN?¡À+"ˆ¥v?¤b¿ÐŸŠ?Ž+Šå¼Ð'?Äþ"–wØ&?ŸŒQ|¤84FGL J0028.4+2001¿éè5fZPÀEAÑöy}À9‰þçÒÑÀ<B_•'Í@¹T
¬ç@Þ=½Ð°‡?±ÜæàÊ/º?¼l¡
ž¿@Ôøš°ðÎ@•wO>'?ïíKþSý¿áH€Âˆ%S¿ç{š—¿ãðgȖݿîÊˆNî{¿ÉxN…ÊðAGNfsrq3FGL J0028.8+1951TXS 0025+197?漣"0,?ƒC.떹?R5íØ_g?J%ñyè?"tv?iH?'P¿µ*½?ï{Û†+?'v¡¥x?PšÔ½Œ?iÀŒ"?Žõà†Ô(?ŽþßDÔn[?ï£WÜ›?ƒëþÞàï5?tæâY¶ð4?kôƒw±?˜±ÜnP›?€ÂZöH ?ï¡Œ5ð?oªRÖÈ"?i!ŽôR@-?Y Õcxò?v95ohÙ?hÌF§[;ò4FGL J0028.8-0112¿ï46φ!ÀOÁàâiÀ;f؁5õ…À<œÉÄÐo@ 	{XæËü@ Ï[†I?ÏèEú
G­?wS¨ÀöLD?£É<quc@ù'#V?ïþž¹"¿èœ³sӌ¿é!P|ð§¿ÑÒ¸~âH¿â³'ÒÓø¿Üj¨ À€AGNbllPKS 0026-014?ïÅ!Vîpx?tYó–&Ý?*á!3¥:¨?'ðŽÚò®?|˜K*š?sÿã†á›?ïsuPt‹À?' ßÙtÀº?Laì"PÐ?^ñ…¶Xå½?±Bâ
u‰?'mØ=
` ?í¦EÊ³?•xIñ)ë?p÷Ý
#>?_˜½tÀ±?±¾U¨Ýø:?"‹ÀÚ_Ít?îy««W?ŽœB|w	¦?M€qÝ{Ð?Aº[ÊÕi?§ñÃô?Ž¤ÅõáÊ4FGL J0028.9+3553?‡É¹¬ewtÀ:ÁòfºI=À:…ðÍ]…À<x4Ô#&@Ržý0ÂÁ@"*ú?Àv\¨¢v?"ib''ž?ÅAÓ_
+¸@ô1ÿ¬s¿¶Là®V4¿âcK^£#†¿è𠬳R¿ÒýcÃHê¿ëGÝ^ëGâ¿ïÿÐÀL`×AGNbcuGB6 J0028+3550?ïE€dwW…?•zAñ­?es»Úl‰*?[»§"0"?"¡{õÇ~?,H-׈§?ï³$MÕrÎ?"[mžjêÄ?0 Q#bÃÌ?Bî(rKøÚ?'µêˆ5Å?ƒç4Öã2$?îÁ!ô:¸?ˆ&í`:Ñ?tüdUûòF?lLñÄ[6å?¡NT1˜†L?…¦§¾
Þ0?ï"=s½6?láuó©I?`]'®aS?Ka
`G^ï?†ÙBe)C?j¯_ˆÅ4x4FGL J0029.0-7044¿ä ÖWm­¶ÀG"—Oß;À9ñÇ9åÔÜÀ<|"ÿ‰;@jÆm¸@k›v¬?·»Z‰Ž^¨?¢ÿËÒ¦Ö?èfÓP0š@‰UC©M?ïÏ8''
¿æ_>ߎÆW¿âPÿÌÔY‰¿Û+ÝÿO+¿ë‹Ÿps/£¿äýÛb'ÆAGNbll3FGL J0029.1-7045PKS 0026-710?ï¾K¡áKw?rÞØé¨wç?Sò";A"?H"ä©è?{ݎ—3û?qP̈́÷[Å?ï²jåȲ?†l	ªÙ`)?4ͧ6´Ù?T*aÉqå?'¾Ù"˜2ÿ?…=v½}ŠJ?îºÜêNŠÆ?¸ñ_™>e?‡óc,Ké…?†%&À$?œª± ²r?"Ĩ‹[o(?ï³^͖
¡?iÝJq¬Ò?[¥³+Ûz?Hq
xDí?g,jkƒ?g§5÷䤳4FGL J0029.4+2051¿ïnŽ#LhíÀDÛG"#À;e‰˜š–À<¹"²²o@"töL"?öó•Þùõû?Ö"ˆô'?Óq"€¥×À@' ùà+N?ÿjDŒ¡äl¿ïß|7‰¿í8Ô'4!p?ìpéý_;Ð?ӎ˜ßŠi¦¿àXºvˆóY¿n(™) ÏAGNbcuNVSS J002928+205332?ï]³sù˜?ÔÆåè
¤?O~SŸ%?F±r?ê B?"Q5Ž0D?@F©ûÏ?î霽èÒ?šU…Kì\E?YÁï³ì§P?h¼®ØN…? ˜$±B
¤?˜ÇIY?ìÏïxXå&? ‡`5øD?"åì-™­?wƒ"»,­?¶ãàŸ³#˜?žÊò"ÒV?쁫¢¥Á<?§QÈ"Ì£Ä?W"€çp4?Vþ
~$b?»"'ØÎX]?§>ß"o`Ì4FGL J0030.2-1647¿ãN¢»^îÖÀS¤5"_õÀ:YÚ´¢À<\ãW±˜@ ŠÞOV)'?úB`²È>É?ÁÚ­àùT•?Á+"V´l¯@—ãÓs@g[¢¾Š?ïÛÛÞb¡`¿½ˆGù黿À´±øàüÛ¿Òµ(kY¿Þ×e­ê¿ÖN²?­¿ìAGNbll3FGL J0030.2-16462MASS J00302045-1647130?ïÞ.é£Ó?aR tܶ?5@K, ?.àŠAï)ú?o0ö¬?`¢åŽ 8æ?ï²ïóÄ~Ü?…Š±}ñFw?2êSÜø7€?J7!t^›}?'¬°oø‡?"ÜÍ/è•?îÅëª=Ú?‹öaÅ>ô4?g4à<ԓ?XÔÎ÷Ð?¢<cAŽÙ!?ŠÖÌ>yb?ï·!ýÇÂ?'P·8½_?KO±iv3ã??øDЏ£?žŽž4ûV?öM8˜¬A4FGL J0030.3-4224¿ïû}(8ÀR‡öý!ÿ.À8â'­ÄÊÀ<1˜F³B¸@¾èÈUï¡@å|Æúü?£Hl!ޙu?ªCŽJ0%@?ÞèXD@u9ÉOiË¿×&F{9‡5¿äúNEq¿ç3SÿÜn«¿æœ}ώž¿î":귙_?ÆNÖgUN¼AGNfsrq3FGL J0030.3-4223PKS 0027-426?ïÑST=?sbZ‹âBl?FÀ¿­ó®?B<ÜTßö«?tšd`—k¹?r)O¨(?ïlY'£Øƒ?©ôlhqµ?qÜÒ)+Œœ? 2Ì
t?‹ûMt{?˜Þ ¯y?î¹Y]?"¬x07#¦?yfÐ9?y»m³Ì«?¡=®|z4ß?'Oþšvx¢?ïÍéüM­Ü?h-4–{ß?`dÐlØ;?YÖXâ8ò?pؙËr¦?`ï¢Ô'–O4FGL J0030.6-0212¿æ"õ»áöˆÀP%‹'¢À8Éõª;¨MÀ;ã{ÕctD@—ä´,@e…—"?§$ñž_Éa?Àpü}êg@°y=Ùc@XÕ
¥?²р)ŸÐ¿àZÖk­Î¿æ¯Ãzm"¿äqêÉ7¿ì"C çU¿ïÿ%¯¼ñAGNbcu3FGL J0030.7-0209PKS B0027-024?ïaǗ¼aã?‡û¨Â‰îw?{_æW#?synŠªÖ^?‰Þ•»õÃ?ƒ;ë¡íD?ïÍ×@í²?ñL©Sï?3YLÞ Ö»?QÖV›šH?x:ÿ'§ä?€êóMÆ?»Òí£?•2¹Áz%?‹ŸsϐϦ?…KŒW-?nÙã·?Ñ°Ûw?ïìl*Káï?RfìY%?.ÇMD¨#?(îN^A£?a§`ßÜuï?PîjºÞ­4FGL J0031.3+0726?Ýtª7eÀKŠýq?À:è7Åi+=À<•(+˜4?@ €³¾"æ?ý\\ø(›*?Ç/–Æ€'q?¶/O"ýÛã?ðœcÈý4t@…¼¿äqN õC¿ìàß8³¦?ãE—Ne¾¡¿èüᛐë?™<ä"Eí¿ãÕàòž™AGNbll3FGL J0031.3+0724NVSS J003119+072456?ï5dw…¹?•ü™Ä–!"?Dè£
#TŒ?>Ö)Ci?žÒX¾.,?•Ìquaw.?ï'È'èÝ?qeš×Û±?<…Úç>0ñ?T õå[)?Š•_Ë×2?‹Ì"MŽ¥?í£œG2¶?"ïóéz?r.òŠOýp?b¥?}Jв?±À/í!jw?"Kø±í9?ï
^e{?‰$Ü{ñ³?2ÙÍfvô·?2ø^úAk?œsLý²t¼?‰\Æ4FGL J0032.3-5522?ç!¢œÍ€§ÀNÆE܃#6À:MŽz¦^À<|R¢dCv@(W·L@ó•$Ý?¹JÔ»?Ś"U•]Ë@	Ëþp³Ç@¶|‰"g¿Ç
G_ɔ¿ÔÍ×ú'xë¿ä¯JÛÆdÔ¿æ+|_÷âO¿âVlSq¿ïÿòÿf}
AGNbcu3FGL J0032.3-5522SUMSS J003210-552228?ï´QڅS^?³.Þà¸?G³9Iìh?A¥;?pUÊg?³22²¹®›?ïßã×Bç¥?vj59~þ?"×ød[:?DÿD'¥?núk='Ñ?u¢våâP?îÔ½·)SÓ?‹›{{Ü?€pj|…… ?y	ƒÔ÷£?0ܒÃ
?†%g¨pu?ïøË°â…?8ùÍÿ"–?H"Wܲö>÷–I€‡Ê6?K¼´0n(?8"ýÌFRÇ4FGL J0032.4-2849¿í6S›ðÀU^c^J8À:ã¹L½GõÀ<¿×ç³ @»ï¶ÝÍ@mnÛí÷?Äy™ßd©ù?·JÌå¤?îè³³ S]@-½@gÏ¿åÜȝ¾|¿Ñø%?–¿åÔdcP¿æ#JóCY¿é¥va†,Õ¿µËÍô?,'AGNbll3FGL J0032.3-2852PMN J0032-2849?Ø?§Z1ZuO?e;ã2µs?Y»§M\Ô?¬°Ã·4?§¼Cñ?ïWªÓU‹ƒ?œïLí;Fî?Po"JÎÛ?gs˜?"µ]	âÊ?›j˖Pí?í­N*8??"–gû¥?"朕ù?s–œ5 *!?°ñÚº0S?'<¡6 M?ï…&Ã؅c?tŸ
›]N,?Uö›?H³"•€Ç?‹÷)œ†^?s¼â§t4FGL J0033.3-2040?½XDq–g­ÀT•zxl"hÀ;ʦ—®ÞÀ<æMú^Ö@!?Ô¶P3Ÿ?ûØdàTi?υ˜…ÈVp?µ·@Hšx'?åD¸aý–?ø‹
ë@€N?Ç#v|´¬¿ïþµbLü2?ï˟`Xy¿ÄðáxÚ¿ë_÷auæ·¿x'Úì'ä~AGNbllRBS 0075?ïwjQ´ëü?"³7l¬ÄÝ?Aô®äõ?=©àmµ Š?ƒë\?"Pe·v°?ï[‹Ð¸?•ŽõP¡Å?Që€'©¡x?`©4U¼ú5?"¶ƒ''?"Žà3ë~–?í²Nf^»Ý?'®öÝÕ=æ?'¤z=#e?zݧ9qù?°ý…e¾?¾ãCÎœ?íF«w<3?¡Z	™Òc?c†#·hÞ?cW·ØŸËF?µ.s-q£? Ê3çc¢4FGL J0033.5-1921?ïð[DÐïÀTMäÍt'yÀ8<Sz
ˆÀ;Pv'¤‰¸@p0ÙÒá?ùꍺß?¢•¾î'Å??²‹À"¦£@|¿ôw5Â@:ÁmH,ê?ãC0×?³´¬š}DN¿ÙՐàãZ-¿Ô!&€È<o¿ÝŒ=ZÔaí¿ÝV"Š‹ßAGNbll3FGL J0033.6-1921KUV 00311-1938?ï¥g'ÝÒ'?'—«M"¯?Uð1ºq½?fÐB·…÷Ç?ƒèIh	?ŒºX{<?I:rB?•×^Ówqß?LƒŒ¡é?cRÀ©#xŸ?tð›Us?•‹"¨*?îq¾ǁŠ?—Egø?…/ىrÅÐ?"wv
Ç=?£˜'á+5å?'Ísþ¥?î©©4þ7ù?"Äu'g?YÔ¨\Ûµ?PS·Ü|:ß?¤–ÇoQ™}?"q<³{p4FGL J0033.9+3858?ïè³æªwÀ7ÆÛ3—ÝÀ:h9Y½áwÀ<v[€YW@>|›Üë@Q«›úœê?Àj˜^D?©þñÀª³%?æíb6V@
¿Î÷õD?ïü¼ž×F"¿ãÆC{Ó¿å+$ p¸Ð¿çÕ)ÈPfJ¿åŽmìl¥¿èޝ´K!AGNbcuMG3 J003408+3901?ïån)~œ?hhÒ¹l.û?=ŽN'ßÿ&?cá4–¯£?fà¯´d»?^{T›?ï²Ï~ó»?'[Èü÷W?0™‰À×??¯Fàjù4?'ÇSúp‹X?»äò Ã?ï'hð‰€Ì?}§9ÃÚ?h—È…›çÿ?Tˆû½È²?—ÿèÞik?{^‹*=f¶?ﳅõŽ·R?fQ¸úП?WÈy£³àÀ?DÁ"ˆåÈý?€%sgÛ¯Š?d<<¡Ú²¡4FGL J0034.0-4116¿ÑOɹ>rÀRÚu%F
¦À:}à{Ö:À<|Ïç/O@èOiõ'@"s9³õ?»ö•Žòø?"p?Ùð??Õò,'¿ãZ@‡æ¦'¦`?åÉTb,ðÏ¿åyêPì¿é'Ò§®/¿çD-÷Š¹¿ßg49eý¿ÜÙü€n¥OAGNbcuPKS 0031-415?ïÍ9=sÙ?rKš5G?EÎpú©?9¦AÕ!ë ?v©¥Áðô?qz'm1B?ïÈlÊ@`®?€tI>˜t?/{eS?H‰ž›m—F?zч£.E?[5à?ï41 Ùà$?ßÊlè€?d¼Hºé‡9?QÈᬲí?–âRÍfÊm?}ÝÖ6V?ïà¸D7Ê?VkéJvà®?-Ùr¤éª?!΍¥£YÜ?mi鑇×ò?U΋Y2´ç4FGL J0035.0-5728?ê˜(ÒuòåÀMÂDú<À:Ö-Ç©­À<—üñý@™ƒlÜw:@={ 1ί?Æ¢*cÖ¿?²PßkŠè|?é5Ü@W@"½a4?ïèËùo˜¿åªqѺ¨¿èMŒæ,ð#¿æ×ÔÓ+‹Ÿ¿ïþÓ°Üá?èÁ'e±ÍAGNbcuPMN J0035-5726?ïç)Çé?`£KÚBfÚ?J)¡G'?E"œq¸"ƒ?bbЛKÏ?\U1Ñ¡T?ïYÏ"á?"ü¶ƒÅ?V,à‰á­?eAƒ•?"zxñS,?"…ZyW‰«?î;û;IW
?/PLjÀò?}Ý~C%¤;?p6¹9N??¨"œƒÚÒ?‰¬»©@B?ï}' ÞQ'?u¸ÛÏ)?k0Þ¼ÐhÖ?\'ÂË¡?‰ê7®?r.¤ª.4FGL J0035.2+1514¿ãŒ7ÐjªÝÀG¹‰a=1ºÀ90õ üÐÀ;¾mÏç3€@Jz'ýö»?û{fX#­"?®Œæ>.û?´Àû³?2@	QÁ
{é…@
ë±îO(‡?ÚqžÞ|øy¿Ø‹MÜ+åa¿Ù8PϞ¹¿Ø(.½'¬î¿ßqÂeؿṈý•¨AGNbll3FGL J0035.2+1513RX J0035.2+1515?ïÉf"oz?nKË뮧û?ADôÿd	?9XRD'°?y$2I¢Ì_?l¥*Ë?RAi…?'.àÐILÃ?D?³Aæ?UC³Ü|þŸ?ŽŽ²{ªj?†c}aҍ?îú°bB¬›?†nku).B?pü!ôÀ³õ?hôøøÿ°?œjë:z?¨?"^iV­?í—ØV•h5?—¨›&EìÚ?dž¦ö·¬Ì?Qûá
¤f?²œHŸó?—¥©¶s½±4FGL J0035.8-0837¿â;"ãæދÀQÈéᰉ À;[ø–2æÀ<´"Š‹ß@+2w÷]o?ÿ˜òtý?Óâ?»+åŒ?Їç^j?úEû7Cc@Ó³#Ñ¿ïý?üoQÇ?î|r!/¥Š¿Ý"m?ž{¿Ö3ªýD8ê¿å÷C~Ý¿ïüRáÏ=jAGNbllPMN J0035-0836?ïÞàïeg-?cÐ÷i¢?H>`Õq_?A¥*|fÈ?kx"#vÞ?a"¶Ë?黎@Ë?‡™#L¦?<Š03BS?R€èûvƒ?…yg:Vë?†…‡dÓЅ?î]v Ì1?ŽQHÑÓå?|ߢßaÁ»?s6öø—Hê?¦Œ©—SÇ?Šù>CQŠ?ï)Gó±Y?€á,¡»!?X¸a¬u¡?KaYãÀ¶?™VO
—?€'ûn>84FGL J0035.8+6131¿ÀÖÀ…ZŒ¿ô­6À9«½¿é{À;ZÿÁße@gˆGa¾a@
{ 1ί?ÇxÐvO'?¼Š"AeÐê?ô¶Ë8x'@
(ùÿ
È?ïÿǀ²—í¿àJú¿ú+€¿è—Z$8Ä¿äöö6R¢d¿ïúú!™­¼¿ë²u"–ØÊAGNbcuLQAC 008+061	?""Šõ?¢È¬‹Jq?MÇi±tH¡?LGÆÃM'?¤é"?¢‰æ‡j?â	¨Uì"?Èâù ¥Â?nX
Y6E–?|77šÀiä?Û±š¡ºn?Ⱦp¶åÈ?èҍ¹Ëk#?«¨Ãp£Š|?˜†È'™Lc?"à‰À*t?ɤð)æ?©|ìµÌʯ?è|^(ô?£ °F»&@?–Ù¢Æe?}ìY×<µ?ËëÄïf?£›G²™4FGL J0035.9+5950¿Ÿw)Òö<ÀÖCEÏíéÀ7ñûš°À;B¬ï¡
@ $|ÍÛëy?ú•†_*2? bGÎ\š?ª¸Å-ò@
ø¤™§ÜR@'"ŽJ[?ï° F\¿Á.ÃâÃY1¿Ý­êžïÄÉ¿ÑÓ
X®ÿ¿ÛB?•—,¿Öîï!
'©AGNbll3FGL J0035.9+59491ES 0033+595?ïyÀžhP}?"j£Ã"a)?:zþ—ЩF?4˜/hoS?^8–­©?"Xï]Ä?ëìm-Â?ÂyÒO/Ý?F‹°S">–?`"¹Õ4`?À7¿òõd\?Áüý³q?ì"çÑÞÑ?£ž5ùÑ?†¤=gËØ?{t'r¤?¼9Ä–u?¢3?ïTñköó?€ñVXP?PÉ–ݏ£?C²ðƈèô?"oq	HÕ?€¡âE[4FGL J0036.9+1832?ÔzBWN¬ÀFÝ/Ÿ¾À:Yºû1À<n}îBh@g*&š£@'L©%þ—?ÀCW÷ã§?¼Ìõ''5?ûz&6Ën@ªk­Î¿æÚ³ì+¿àú®/«¿æ,@Ъ¨¿çÞ¯°î¿×)9_G8N¿ïÿÁìžú,AGNbcuCRATES J003659.39+183203.7?ïʇς@Í?©Ó›hš¹È?;õLÍÁ?j—ÑœÞù³?xüÇÊÈP?¨*Þ\S 4?ïÐÖ&«ð?{?—ç¦â?#p™g$?:Èâ½`±§?wT"‡á,»?zg¼×H3?ïôð*?ÏŸ°ø©è?gÙȧWÖ?UÄN‹þ?šDMÝÞ?€Í ¦µß?ïïè/Ò?Jï²î|œ?}®ž]?à®ÆŒ"¤?_'Ñ»q÷ë?J—g§š&4FGL J0037.6+3653?ì`Ÿ"ŒŽ'À9ä—{žÀ:ÌÿؒӭÀ<t1rhÓ(@ÆXIî@$UšfH3?ÉÌS•©J?»zàÆÔ».?ðÇ#Zx›@Dt€ª_¿í¾ûˆ¡ú'¿ºÕ¢"C¿åÑÁD®[¿ØkYë-àä¿ìmˆcç0%¿ïÿÃßé47AGNfsrq4C +36.01?ïOpLþP?‡j…F&hi?crËZ²B5?\ˆoÛ\?"£œôè­Ó?†'Fëkv?ïƒûý"ž?Šõ¾­ºK?@ž¼1?P˜ƒCpû?Žϒ3X?‰/äW¯âI?íňÝ_iŠ?"Œ àjçÌ?‰`õpç?ž?|PÝ£ï'Î?­O4Íϗ~?	~…ôA)?ïeö¿JŒ?€û&Ì9#?s{\õ¦Ô?`µ'ÏóäD?šTaPÙDÃ?€ ÚQ\QG4FGL J0037.8+1239¿¢®X½bIíÀI
¥¤i×4À9€C`§à"À<+»Ù_'G@¶I'uç@ÁªYÛ=©?­²ÿµò¿rÔåþªä?ÃÓ·79R1@z~ædùT?ïÆZAêÜ¿â咖pn¿ä›:]ôÒпà+Ôßë¸u¿ãÏß Œg'¿ã]åÄ—gAGNbll3FGL J0037.9+1239NVSS J003750+123818?ïÅ{|.ž?s–ñ=Žšv?7Z0÷*[?/g¯SÃA?{̞ي
³?rú.,"®Â?ïӍ­;»ä?zŒðñŽz¥?Lʝz?3ŸôçNÛ?u¿ö7­§Ú?yñlÉSî?ï0q"Ã³?}ÁvK?f, ÝÑ©?QxµYœ¦?—,;^ÏP?{ÍÒBæó?ïÞ@Rçs?VŸaáëOÑ?:­—•´5?)— Y›?niû
b?U5€®¢kË4FGL J0037.9+2612?ï6›gÏòòÀBI/Ÿ¾wÀ:×Dœè³À<ˆ')ó@+QّG@ì楻æË?Ì.sEqú?Ã'À²7J?óŒÙ|Þwð?û҃Ee¿Û@`óJ:¿à'È>Ȓ«¿ä¡wÿ•÷Ï¿è"J½¾g¿é.†%HŽå¿ðAGNbllWISE J003719.15+261312.6?ï&;É·2?"°i[8r?^*ÛXi˜?V^ib^# ?™UÙ–èú?"9B¥žæ?î#à6ϼ?¥$™}ùÀ˜?qVÿ<¼?'¿ÚXH*?«£²
ï¼²?£Ö&tÖÌ?í®¿_-/?"&	¿ªÛ?Š¥:=5²?}WK'5?®vU'=ߚ?ð~ñ«â?í™ Š°.?'ÞwÛì6t?‹oSJü^Ÿ?vQ9/›5?¯'1$•ål?'—£¾ö"34FGL J0038.1+0012¿ëýò,5p®ÀO<±î$5iÀ:úûö†À<_zù›añ@»…øÒå@
¥|üªá?¶	Ê?eò?–õxί?âp¢qON@ï72œ4¿ç•¿x¿ØCûlóHb¿åCW}ÀJ2¿Óîᵒ¿âvOb=⺿â˜H+ü'AGNbll3FGL J0038.0+0012NVSS J003808+001336?ïTæjÛ?Šƒ\"x¥?Wœtƒ†§?JÞ8kÁ8ö?")fªl'?‰)¤€­?ï'psØñ»?ªVöPÞh?Fñ»{
•?^ЮÞ% ž?‰ôÇRè@?‹À›ßíaï?í`S.ý?•xfÂV­p?ƒEÎÈ´´?vïT‹?²‰½Ñ¶üŠ?"Ï"šÛ?îy÷I4}.?Ž6ÈñÒ2?rh~¬ø?b&͊+n#?¦¾\â©H?ŒÞ¿ˆ(€4FGL J0038.2-2459?ÞúÔaì""ÀU–Y_í¦aÀ8ùþz¾ãÀ;ùž$BÕh@8ÃäpØZ@Q¥Ãsˆ?¦e¯¡º?¶ÎQ ï¿@aƎÅ*A@žÌíY	\¿³ÍlÚɺŸ¿Û-+|…Œœ¿äï4 #b¿âˆõý¥¿ê@N¤©¿åó4«wªAGNfsrq3FGL J0038.0-2501PKS 0035-252?ï&~ZÜX?7Ìûƒ?V˜í"ñڙ?Sv'à)w?‰cB¸ª®ä?Ø´êŒ?ïÊÂŒFd?ˆ\– ¯;™?%`¨¦ëž›?A÷ªÉR?yó—ñ¥p¨?ˆÙã0[ ?´ÇKÀ?"C«¶ñðè?… ëÚ?nr¶:*3?¡Öl¬Mz?'¨"LƒN?ïþÙG?"Ò´+ëV>áWîo—ÿ~>à(' ]r#?.铄•"Á?"öûih4FGL J0038.7-0204¿ç[w4àÕÀP0¬![š[À: ñ68¡1À<F"—u@Ëßèˆj@÷ÇÀ?Åd¦¹
þ?̟6çrÀg@öÇd­ÿ'@óœÚ
οËB#;"Ü¿æBM'iÒ,¿ëÍQŒºŽ¿ï݄?•AE¿ïž©£Ò؀?Áþ0\"*šAGNrdg3C 17?ï'j%[`?ˆîG\Ÿ?g‰Ƒø'?dÌQz}!?…ƒ3wƒ{?†±˜N/F?î^Eù¬üÏ?ªjÙSRý?ƒ)Ýç@ÿ›?Ì4HQ¸/?¥Q(ë_ó?¥¬ãå~f?íCòòÂö?¡A Ûó?'æ.Cø ?ƒ@9&᪍?²ÄT×kÄL?œ÷i¸iñ)?îY—Æ_n†?ì5*º•?ˆp»¢õ½?wƒr5š?¤JTÖ`Z6?Œmëݦ»ê4FGL J0039.0-0946?î9{"Ôk…ÀR,ºËCÀ:#ª–A…À<f=°d·:@é3þà\@u{­ˆ?½í'þŘP?¹PXÝç§?öüºÑ!Æ@û!'ÌËË?ïÿmh¹&þ¿ãšQ_™¿¿é5Ù L£¿ètSß{%:¿ïÿñ_{'?í(#ÕÈAGNfsrq3FGL J0039.1-0939TXS 0036-099?ïìC§n È?[Z÷ٚã³?@·Åz·—?@²™¶ü%?_ÁG?Wî9úIC?ïGóž-Ÿ?™9Ž£
A«?cN{ÇÚÉr?uìƒkH?"—¼ÄÞòÖ?–1'ûÃ0?î"Vî‰×à?Ž‡_ŠïlŸ?{÷8Pþá?u:8R)ð?£;ª
^â/?‰ÓÎÃqT…?ï‰{³1©L?v²±—?rd‹w:@?g3+%¯Wö?"Z`íÚ?pð[àkò4FGL J0039.1-2219¿ã?uù×FùÀUg8}¿À:…®Ús~}À<o­é¿@ ÚÒZ*mè?ü(—ξ??½
díj| ?sUÙë9I?¶©={‹'™?ÿ–ãìÎõÇ?ïàYÜë(¿Ö8è^£¤_¿Ôb·ðœµ®¿Õ1fªY~¿ãZ7ÿuÁx¿ÅíQ½ƒAGNbcu3FGL J0039.0-2218PMN J0039-2220?ïnü}î?V!ޓ@?K4ÌȉË?ACA¨ç|?'FÉáÿXr?Œ´©õìAG?ïA´†}Ë7? ÇÖK–U?PڕrÏa?g=¢z¶Ï?–»ÅÙ£"?Ÿß"°;é?í–ýYÒ×?•OñgIÔ?y\æBsl?hè9£^TO?±²F՝B?"po¹«Sz?ì×ÌHQ·Ÿ?™R#õ?r•a+79?aˆքj?¸G­O?™	ÇÅþ@)4FGL J0039.1+4330?×*²zTô"À3M½ÙßÛÀ:¾ü‡7À<žÿ%­B@yl®)@
  ôØ?Äa1s?'½?Ú6bÂö?ýàõþõ>@	·"W`9&¿ì²ÊÃQ-?ïùZ"¡U¿á­,ˆõ¨¿Ýe¿cØ¿à/³KòG¿ïÿ8"†ZAGNbcu3FGL J0039.1+4330NVSS J003907+433015?ïó÷"¶J?M±èžøå?@¿ïÓÜ.Ÿ?=©Ð®qDé?OaýRû~?Eœñ*ª?ïºÔsw´?'/¬·Ø?4"1â'Ì!?Edi"«ä?€©Ñ¯
ü ?–,9>Ð[?ï'½Ë¢vC?€šM‰›n?föÕ¡é9É?`ÑS­gk?˜)k×tq?é4+'•?ïs¨
¯SL?s#ãç÷'?iNÀÛS?W;;D?ŒÂL]j؊?r½‡ž²4FGL J0040.3+4050?Ñ*e'潩À5ü¼ßï¿@À:¸Ø£š¤À<zøØÄQÔ@!A߇O?ÿ¿ "_õ?·[±×~·¿³0M¿jRs?û-
ê¤N)@b14?èöIØÃ{¿â6M™æÆs¿èê"‡¿R¿Ö^¿à12I(h¿Å"§ŸÁ¦ÔAGNbll3FGL J0040.3+4049B3 0037+405?ï[¥·Ô‹³?…Xb¿Sü?T6Ò7|`ˆ?K5ù¢Š?"GÛáöÞ?"®9.ç?ïQùbGŠ?"çÉ#ö?Pa9ƒÀ±?`ÂIzœ¥?"½²ÀÒÌ?'ñ£ˆY+?îTõ°&<Ç?'%)öj;?iXó³!ÎÛ?U-ñK–§?©Âjµ?'è…b?í¯§ýr8?œâ?ø…p?zà¡vÃ[
?n²î'èU?µ\x¨¨8˜?8r¿—4FGL J0040.4-2340?ĄMóäúÒÀUo@öjUÀ:˝_÷·À<š/²u2²@ÍÛLlj6@v¿yýòà?Ædô5òUH?ª"Ù…xO?ãl Åre@3¶-y
¿ºÔ뿬'ç¿èk"\Ì4¿ã³A
ŒK¿é}ÉÄڐ¿ÉÕdK3'¿ïÿס<%JAGNbll3FGL J0040.5-2339PMN J0040-2340?ïrq¬º¯™?‡'•+h™t?SsÉï8¬?K÷wËYâ¥?zÉ±9J?†üMò.?ï‹ûÂè"(?•ë­R™qÍ?B+̐1N?TJ–æ-M?‹ÞR|õ¢À?•.6PtMÂ?îi:²q?€WìQô?pÊÍ?¦BD?eä9&­j?§U¢¬êp´?ŽŒÎ">—h?å§ý»?p¹Á<v  ?3R¾Â»?+úS¿Tšá?†ø𥺀±?p©ÔTÈ4FGL J0040.9+3203?â+©·§>À>Ä(äû—»À;ðR
À<]J]ò$@Qmª'†W?ÿ–»cýM?ئËEäß?àEÜMsPZ@ÙÂbæ@€ðâUË?ïøIóiȿքÖ~|\È¿á¬btx¿äÏìÂ5š¿ïØl:¿å5{!ŽAGNbcuTXS 0038+319?î\F¶g?¤§ÜÒ»³ò?|yØÆwõ2?z2윤G?¦¬dʑ4?£F\£?퓓á,ž?°Ø¶˜sÂ?†Z¡]{?˜=ð¹)V?°Ÿõ¢onÝ?ªªÏ0(¦y?ë؟y=Oô?¢{šHÓï4?¦²³«h_?'ª©ƒŽ?µáª`aPÝ?›¤OµÀ?í$"â¾SG?"_ɾ%E?‡8ìBî?y«Göš{¿?³ô^…#?'âǘׯ4FGL J0041.3+6052¿åðÓÈrí¿ÿƒòÖKÒÀ9šN³Â9ÌÀ;Jˆ0»‰®@5T#sø@ä¬å¦¸f?ŲºÒÏEM?áúˆÇº>U@‡žYòº?öY0³Q%·¿Þ–ý]
w7¿Ë$úì.'¿èÕÃ"æ¿îÎR]ðÌ¿ämÊ=¦S¼¿ïè/>\;AGNbcuNVSS J004058+605407?Èwfø°s?Á9ðIö'`?ÑHh"œ'?ƅ'(½~?á><1ÿ…¢?Éï¬ìÕ(?ªUÊ´"?°Îè…
/3?ÉY'?¿*#?ÄüutuÛ?è?ÎDÿ?ÄÝږO+?Ìø's=´?« ]¼ßPŽ?Ì¡]т	±?¯vC†—\x?ᦺÂ®'?²
\/?Š1­[WQ?v'
y7?â KÝm?¿PPŋö'?ÚíÚÚK-P?¾™šù$®Ø4FGL J0041.4+3800?Æý±Ï3ÉÀ8ÑüÁr&À;ŽK^À<©G_ɔ@ ÉfI
5
?ÿÉT!ÀD(?ÀU€ÙÚ&¿­§¤|ÕX?ï0\S½í6@½ý|(?쀏qøjà¿äŠ:N¿â֘B"пä÷bØ<l˜¿ÕœøÞbK¿Ä1ƒìÅLAGNfsrqB3 0038+377?ï4ÅV§9?ÄíԐZ?[ZSï\?QY
å7Ä?—±´H,#!?BˆŽ§x"?ï,l»qpÇ?œs?sÞú,?UÜäW{à7?i¿ciØÂ#?™šLZ)2?šœn"Eô?íè¡~n;.?'érͽ &?rð'ˆ[š²?]ʖ6‹?¯ÕÈÙ¬?'!"ÉÁ?íÌá"s<?™¶
{²Ø?gd둒²6?aWfDpC?°ä™š_Д?™Rn}ºmÑ4FGL J0041.7-1607¿âÃÃÓmÀÀS±úëÄ	À;±¨´¿ÍÀ<ÜøÆOÛ
@!ËXàÁÌ>?ú;´4çh?ÕغEºÊ?ÇÉFZ'W‰?öIŒ\`S@DÃàj
?Ûö'¡þm?ïúeµ²¿äå\{+‰¿Çܺ–}5¿Ë­šW"¡:¿ÖÖò FAGNbcuGALEXASC J004141.24-160746.6?ï2Ý-…ò3?'E.)Uïí?_›Š×Ü"?Y^à'!w?—ª¡¡Ã÷•?'­ßM:'?ï™p·
…?‹c'õ€	`?D$õø•ÀT?`á+U"½i?ˆa'ÞsBù?Š>ÒPªr?í'W.X¾…?•rãx Í?rúáT˶?bCí­ê?²E˜wíYè?"Lè\Ÿ?îDe=_Ê?•oxPÿZ£?Lԏ^']?Mq´özÃ.?¦¸iì‰?•q–ˆp14FGL J0041.9-4702?ïNÑ«–îÀQ­À˜$À;ã‰>ÃÀ="ÏÝù@ Ÿ³-¿Uì?úõp	}WD?Öí!zN%?ËD&J—}á?òò<ÈÞ*Ã@hÍ¿ïÿü¥¬¨¿ä¥AØèd?ïÿê›ê¬²¿Ýó"Çz¿áY®Çÿ¿Þž¼n/ÞAGNbcuRBS 0097?ï×òG¢.?r)_¥ü	¯?5Â{"Ð?8¤ä(¬Â?s!_,&ð?q%]ˆ³.?ÜOhi?Pi3?DÍ~í¯Z"?\^»º»¬Õ?ˆ
°ýJð5?>'Vì>ò?íòÃ8"h?'IlÌ?~ŠÙ3UB$?/«\3'¾?­t¦!H?ŽNIƜW·?ïn©""Z—?~›‡Óz?3Gñ<û?2DᖏB?'Ý­§o¹?~JŸdµ/4FGL J0042.0+3640?¿gÈf5¾ÿÀ:)/ ×{|À;ò×ùP¹À<Fyaî@È)NWüÁ@ç';®+ø?ÃD&àêf¿ªñ/؊Æ?ËA˜¦ªy;?ÿ¡W¾'Ý?écànë?î¨ü
,8m¿ëŸ|!Ž›¿ÑÎû%OÅ»¿ßÍã£(
»¿á¶Í§%sAGNbll3FGL J0041.9+3639RX J0042.0+3641?ïaÐÊ#4?"ýëe•œ?Y,h.ØÒÎ?SÅü¨Õîí?'3 8«ðS?"ÑÂÕ½Ž?ï}ôâCÞ?‹q"¼µŽ?D€Ž¡Ã?Søæfñç?:õ^Œ1?‰å¢úú³?í·+uÙ?—1çÀã?téL'Ê8y?b/µ¤kX ?°ôñÛ*ý­?–4ž§`ùš?ì% l?Š$	= ƒ…?'·Ð–…Ñ?uÛúG#=?¡è]'Ç?…ÞK|Wš4FGL J0042.2+2319?æI…ýQòÀC¿rÅz%À:#ŒÍ}À<b Õb"@\*2	h@Ö×¥mã2?¾‰_d¿rF?¾Òo_DšJ?ýzŽ ¿"(@ø­ˆÛ0¿Ÿ»Þ#G"ú¿æ²g'Ñ`¿ã$e¥vF®¿äšŽ:!¿è@*'_–>¿ïߏ@zAGNfsrq3FGL J0042.0+2318PKS 0039+230?î%õÜÎL.?¤Ù¦¹v*˜?xÄñZ5",?vQ"3}?ªˆԊ–?£¸Tè«ð?îâ"g5•Ñ?¡jy¢e'­?b‹ñº"¢:?mx¤»½? µpýh¸? ÜÆl,ó?íáùèª`?˜hùí¥ù—?ƒ')N²7E?u­µ"À'?¬û× (Ì>?"Ü̓'C?—ê¶?…Œ‡\³?"©¸P<¸?l¬‹·J®? z˜mOÒ¨?'Ë5ÈÏy4FGL J0043.5-0442¿§´]ŠÅÀPߊ\å´$À:æ~Ä+=›À<†,:ñn@ š:ë
š?þ Aׁ\?ÆÐ\cÙ`?¤âcâÓt\?á­»úíqˆ@""xB[ð¿ê?.8¿âÑBþ,kC¿ã'·iŽ9¿Ö
×YÉ¿àý­_Ÿ!ï¿ÍïªGfÆÞAGNbll3FGL J0043.5-04441RXS J004333.7-044257?ï"-hæ3?
…2tfú?;åå¦sŠ&?,ò J*R?Žv²RÖî?~¬ÛH–?ƒB´?ŒfÏ(.ðô?>';;8i?P"¶³jÝþ?‹#Š¥y%ì?‹:8×ox‰?î+ê¼½"¿?Þ­LÂ΁?m3ÝQPÆ?Tó?$ꫯ?«n#¶RŸ?Ž¢³ËbéP?îø©õ—?'6
†ºÏ?XÙÔìôq?P—t"ƒ?®¹°ùÇ?'#}ÀU­04FGL J0043.6+2223?ØEFÌÿ2âÀD9‡çÀnÀ;¡"úÖËÀ<'g†!Ñ@†Ã>@=–é»ðÜ?Ò£9UŒ$?·iþ Õ®?é=[?Á¶ï@¾†ù¿ïØ ó•Žr?ïџD~_¿à¢wžÈ·¿ß.8øo¿áéBžá7¿ïþΈ°=AGNbcuTXS 0040+221?ïÛ°WÞ?dÖåÛù¸Í?3ÛÚ½"?-;W°Ò?q2vÆÊ¿Æ?dÓ."¼'?𧻓_GÖ?"éࡇcÜ?-8:»´?B	¶ËS?"¥¿MŽ¼?"9ýæ"R?îs[e¼²´?†¸Úv¥H?q Oq¶él?`ÔP&Ñï®?¦–?µý÷ƒ?…GN†uN¥?ïP?w+0jÿ€?Um8&ÁSÁ?Ilºkß?"¨©9҇#?v¹62﫸4FGL J0043.7-1116¿ïD"†YmQÀRƒ7u¸À:șI—#À<ˆÊ½ÿ@ )Ð3Á?ùz@Ù#¯?Óì'?
?Ñ"‰âíJœ@¢Pr[@}¢×/ý?ïÿŸ¸fä¿ëa¯ÐâÜ¿Ù5 uÖÇ¿Êò*Z~&¿æØåÿùŸê¿ã‰!Q^lAGNbll3FGL J0043.7-11171RXS J004349.3-111612?ïq œBÏ@?Š"jûQ•?DçX;õã?;ó$	ƒãj?'4±¶Ä8_?‰ºë ô¨h?ïkrÉ1t?"sÖÔ8Ü?N¦ây÷?Z‰ç5á£?'œŒÇÈÝt?'´¨lŘ¯?ízÆl<`û?—y`JÊ
?}APâÚ8Ó?rDàZh·ñ?²U·ïT?–'±Íæsð?íA©n¦ƒð?–露ö#–?^.Kª0ø?Tƒ_Áí¤™?µyû\#µ?–Ák{4FGL J0043.8+3425¿Ê¹IÂì¤.À<j|¦CÌÀ8b–›¸XÀ;'U¤wC-@^[/¦Œ?ýÓèPïÝ?¡kÉýQ?ªs‹_fN@
¾•ßе@ýýÃå~?ïÿG©ýd¿Ø\4ß/ÐÓ¿àíØJ¯P»¿Ù·ã܈׀¿âÝÞQ"'¿à°éAw™•AGNfsrq3FGL J0043.8+3425GB6 J0043+3426?ïÕüחS"?s'ñ$óÏe?1<+ã]q?Zg÷³?tŒÏC¦°w?sc"'ÂËñ?ï½%lk?í?®ñ£ƒû?7YfÉkÕµ?Q鄅µ²û?÷³]ÉLw?€¾Í`w?îÈLüçš?cjÜB³;?sҘÐWI?jã›oёG?¡ˆ0{t?Ž}+_ÍQ!?ïµ®'ü!¯?nyÞ¢X­?;´x_q6?.y§	‹^ø?¶·À˜ó?n0å(NE4FGL J0044.2-8424?™q=—ÖšÀ@\¤~Ïé¸À:P"Þ™À<:Dfa]é@Ä9Ö:Š@JCþ\'Ñ?À4	òÈ	?1SW''»?ÐU@0ÞP^¿ßB™¢ÓÔÿ¿á€Ì¥Wh¿èˆ^Þ²¨¿ëÙY_ç¿ÇbT]û2ç¿ïÿ`}™2ìAGNfsrq3FGL J0046.7-8419PKS 0044-84?ïðO,Ímï?\\Ÿ<™!?.ä[1ê+s?)±sB4.£?[…þæْ?[ãiÔÈ?ïºe J™?…É~—«‰ò?0GþPÎþ9?T—c'ŸÑð?€ä`Efâ%?"R;
èc?îË%-ϓP?Œ˜çÊþÞ{?jI^)@¶Î?\r?ºþ(?¡©@r¿ž?‹Òµ7¨?ïãÓÝ&ß?Vô˜¶Y?í™qľ?3
‡ñï?kM'Z
"Á?UÃ;yH³±4FGL J0044.8+6802¿ïR{Lý^»@²{²þÅmÀ9ÈÇÜ$YÀ;¡óÒvZ@ו#SÀ@N
Ää ÿ?¿TWñ?³S¡èÅ?õÙ	†'@éšòŠ «¿ÕßGŽ4
Ê¿ŽXkã=í¿éùù î?¿áx7Ÿ(¤º¿æPqgKh´¿èë»MlšAGNbcuLQAC 011+068?êøn‰¤ƒ?¹Oo5'S?€Çär­&}?vØLã¼Þð?ÃǒD»†?¸ß[Š$O?æv†¡LI?Äë·õÁ	1?'ÃiÉ$£]?§"»º(÷?Ób÷¤tBR?Ī׺l?‰?èMx>ݞ?±~#‹,°n?™Â±éq°?†Û¬:PuÝ?˓(Ç[S?¯û­•{´?誷xqˆÊ?¡LOA,cï?˜ú¦z.±¡?}m°I¿.?Ê5ÍNô¤? œß¯™4FGL J0045.1-3706¿ãQ>܉®?ÀSûί%À9µ@+i:VÀ<†ãlK'µ@çoÚX|@¡–EQBé?®©é…Y?™€öà^?çœAƆ@†¥ªõ·¿ÏȆŽàÙ¿æ4B'KÇ¿çÖø4Y£à¿èå—ží–¿ì '¢ s¿£.üÓТAGNfsrq3FGL J0045.2-3704PKS 0042-373?ïæç>Ms?dP¸yàü5?:]‡3G·?7e*ÄÄ+D?eՖMÌ#¥?b¹Ú'tž?ïÑ;o-?€šiû®eî?0å¹4yvµ?OVm$Ҙï?vp†µ!ÛÍ?Ze­a2y?ï>H…9Ÿ?|æžÜi®?it‡Å£¦ä?W¿Èëp%]?•^`*÷a?{;'èíúz?ïùi*^-?;t=<‰?!¢ŸN€8¿?ˆao —ò?Eò®´C@¢?8µÛ\	4FGL J0045.3+2128¿¸^FàÙKÀD°üó0À8Ýi¸*~YÀ;œñ-Õ%a@¤zŽ¤h?ú´‡Ç	>m?¬º¢}ÃÐ$?³ˆ¹ø^Ëè@ZÂß
A1@žA|Í,?¹Jˆ ‰3+¿Ø/õ;*ùS¿Ùåpݍº=¿Ño¤}£Cç¿â9ʑ‰)à¿ÕT•cT
HAGNbll3FGL J0045.3+2126GB6 J0045+2127?ïì\}H./?[Øqöb´–?–ÇS¦ÅÍ?½Oa'?b®Ì}4šå?[<RxÛ¦?ïËV¾Oà*?}Ãl™P?.Û6coZ?L½×|ª' ?y]È®\ÐÄ?{»Ç^\A?Hf?'"~q¦Ö?smmV߯?n;ä%&¿ö?¢ÚÎûd?um:û(?ïÅ[ù±ôã?g™CÓªÆ?¬3w¯¼?
æ&–`
?|áÄv7°?g}ªÀñ6Š4FGL J0045.7+1217?˅îC6'ëÀIGD#‰À9QË(‡Þ†À<IbI¡4@¼ÇÞ{uí?ÿPUhaQ?¯<òN¼{œ?•(%Ž.?çs÷+E(@ÿz'î.Ç¿ØPQÜÁŒ}¿âI¾ó(¿Þ¯îºÞ7Ù¿à')ÜÓ¿×âš~ñ͍¿ä[³"ý*cAGNbll3FGL J0045.7+1217GB6 J0045+1217?ïÍÔÚAQ?pÏšòY?8wæzÜ?-ÙÓÚ.»?w"{ŽÐïM?ný^銵?ïËlAc÷?~AZºÍøc?(€çgüµ?@tǀ95Û?y¹ÉXĦ?}5wG½?ïð<¶k?ƒ:HC+Q?eþnÏ°à?]\ÒÓF"‹?›*<ƒ?Îö'±$q?ï§f´Š/?oºk^N;??>"¶%¾?01®Zâ¦?…2-Gõ6M?nÁ
ݕÀ4FGL J0047.0+5657¿ïb…ÔêžÀ 2@Äì.À9'RYi'âÀ;áJóCY@Äé÷U @"úC'œý?³õõ d4Ä?½ü`‰ê
@	,žÄ{Å@ý¢Žø×?Ôy™ž÷ýR¿ÔúŒ"¸'¿á»´v"±Ó¿Þ­' ­ßø¿å`s^™¿è fèlAGNbll3FGL J0047.0+5658GB6 J0047+5657?ï¤.+$0?|G*}ó]I?R0õpÅc?NÄ钅'?"®aQèۂ?zlxÇ34$?í"Íu¬9˜?µk',AJ??Ãÿ`"j1?[HjÏ4ÕÕ?¶ÉÐS=žÖ?µYŒwK?íҁ`åÔ?'dŒÚqË?€å"S×Ð?q¼ôcÝ?®žˆé;®Í?ø+R~g?înW'R?Xßà–î?`¥™Ê¬f	?Jƒ'IÏF?Ÿóšûº(ê?€×"çÿ¯4FGL J0047.1-6203¿ãyIbÓ"ÀKˆÎp:ûÀ;3&yÀ<‰ÿæՌ@S1j0Jv@	]"à¤ñ?هö#]RA?äiTpš?ú¡#K^£$@k%mL߂?嗀Œî;¿êŒºùe²¿ïü£õ=._?íSÀì÷¿ïZ¿Ï
o¿íã°> ÍAGNbcuPKS 0045-623?í;£PÜW"?Ã>¢Ñ"g?´0$qzØN?ÃG{¼·?,z&±Ë?"cè­ü#,?êS:óGÄ?ÏImVžl?¼Cvñ&v?̆&=žG?±"´‡?¼j?²°Â;˜ï?ê/@8³êq?¥Ç'Š)?¬¹*ï_?"?–{o*?À´aX†Y? ‹ÙÒË?ëoz´Ü?Æé2%¤?À.÷»;Ɔ?Ç>€Î-4€?šºRϟ0??žŽä!…4FGL J0047.9+3947¿îL~Lƒ‰À7¶o"5ÒÀ9uÓú¾wŸÀ<*¯ZËþq@¬Ë"œ?ÿ1è_ÐJ0?­óÆB"?œi³Å6Læ?ðw_²íþ@»4‰tˆh¿Ñ	£¢†þ¿áHÅ †l¿ß®¬:Ûô¿ßj
 AÿT¿Ûä:|¨¿áª	µólAGNbll3FGL J0048.0+3950B3 0045+395?ïͼÆÓ°†?©!óîÉÄ1?/T?"'û?#Ðá#x8$?x&ü.¨x?©"×zÄî?ïÓÛk¾˜?zFgfLq?!‹±¸ð<F?5hŒMaê?u…ì"7²?y°Ðy¶×?ï*Pj‡ß?~$Ê1Õ/â?dª
Ó
??TCd훺Ó?˜ ±T®\W?|=Î)¤Pl?ïµ[f{¯?iµ+²—?@G°úÎY?. 
áÉöü?¤«QsÏß?häÚb•¡4FGL J0047.9+5448¿ïزކ€À "q›MÏÀ;MHœQÿÀ<¥;Ϲç@#—/£†­Y?ùJ?Ú
¢ñ?Å …œº¿tˆÏ-5~?º´÷ Þ@íšü?ç–º$Sœ?ïþ¡ÆŽÅ*¿êZ^gŠS?âúÎÓ7J¿Ý=–ä]$¿ÆÑ>¶ôô3AGNbcu3FGL J0047.9+54471RXS J004754.5+544758?ì§ñ/̧Ñ?ºgÝ:)£?a5B"{"¶?bÁçÂÉ_@?º6Ìlþèb?º&L,bñ?æozN?ϙÂÊ	 ?MÛ¼øŸ·¨?eêÐa˜^?ÓÀë褻‰?Ï{Èç²%Ž?é5*\Ùì\?¦ªÂEÚ1 ?"ÓKq¾¦Ë?pW¡äŠ '?ÉÞ!Õ|d&?¥ÅðŒp©Ý?íd·«P¦?§-ÚÚW±?ƒÚ±èü˜?ƒ}ÛÁt6?´©" [T?¦1Q¦Dî4FGL J0047.9+2233¿éËÅXHÀD&™Øƒº4À9àGÐy)¸À;é•é
ðõ@H	 <Ëã@åäËÇ?··Rèa?Žá‡Ÿ¤©?ØÇW­eÿ8@UC#Á%O?ç(å!,u¿å˜|··ð¿è¯;Œž"¿â13~²†¿äñˆ£¨U¿ïþÛÝáÈAGNfsrq3FGL J0048.0+2236GB6 J0048+2234?ï󌨜HL?Q+"zèw.?.Â%±(?"Bç[?Uj$®ò×?OÑcUÄòƒ?ïÃ&.ù®—?‡¹Ù¾åª"?'¡­Dԟ'?N·7?™'?}¯Ûá?‡"wMÃú?îéÆKÒ€?†c̬Öþ?pÂÖ
ŽU?aø‰?ž–yìa?"^5
ŠŒ?ïÀ‡;^x?fÁqµ¬ñ?2-k½Ñ'?!ðÊ)¬tè?~™‹"æïw?foë:ËÜØ4FGL J0048.6-2427¿ï+҄zV;ÀUÐQ£"îÀ:×{‰äðÀ<¦WF7ò¶@Dú¦#ë˜?ÿ¡¸·lx?Ä~´%Œª?º5‡Ì<¯?õ®žä\6@VÇâØ'?ë1` (Õ¿ß[dc¿àgN"¢Â7¿á÷7…¨K¿á¥ø¸
"'¿à_`îWaAGNbcu1RXS J004836.9-242631?í.2?š9Iæqý?]2Ÿß´y?a="—6ÁÊ?¶z¤ŸŸ?Â{"òåqÎ?îÐ#rÙ§J?³Æ Â-R?Z©™¢ò?qošQ³k?¢(|T²Ê?³
Èá'ß?í<xû`²? Ý«	:ë?sA´'4^9?]ʑn`´.?´è$W´‰? Û²Ò‹E?íííƎm¬?'{‡;ñâ?k"åèÞø›?\¨"M ¦"?¯hÕ8‹5®?'lÃáãû4FGL J0049.0+2252¿î^Þ`?}ÀCÿU›=ÈÀ:Ýeõ'^êÀ<<À%z@éíÞjY@œ©ïR2Ó?Ê ½šTÕ?¥‹"òe¸—?ÞVq[Œî?ÿ[ˆdpm¿î`ýÀµ'?ÕéxÔýó¶¿é#"¿lçà¿âü	Ñ:׿Øã_5o£¿æ}ÆUˏAGNbllCRATES J004901.37+225315.4?ìôO1á?°$›ºýç?m(Ÿ!Ë?lѤëÇâ
?·tEÓþÖÕ?¯Æ7«è?î"?!š?®^}æ'Wä?c yö$åä?}Kâޏ²?¥'Nü¸?­G…RoºÐ?ì~}ߕwm? ùW´Âb?"ý_{8?t‹+aº?¹s™WdҔ?Ÿ…ì	Ï?ëc|x
?¡.š'Þ;?w‡‹>ØÔ?oBÁûIEb?Ã%–5´)?¡0œõžÉn4FGL J0049.1+4223¿ïö¼5¥ÔÀ4zÅ;ËÀ;*|næg©À<³ÿþR€Ö@ ×âæê…D?üQ¸> NÀ?Ó Iaûc?¿ ãdéº?ï-Ú-Þ_œ@|Eœw?ï¯2Ú˓¿äut¡<¦$¿è$cÂG7Í?"UM[ÊÎg¿á¿m~2µà¿á6ߐðAGNbll3FGL J0049.0+4224GALEXASC J004859.14+422351.4?ï'a|¸lÓ? w±ž†‹?6ƒMó/t?4•¼fë?Ž³†bL¹é? oKçŽ?ïIìyÉ(?•šÎV൩?M2'…FrX?a%}Ǚ'j?•Øܲ°Ë²?"éÌi
t³?íù1bXB?' LÍëÖ?l7h¿VP?Zº®€Ë<?®©sS…l?{£™B?îUAØ¥é™?àh2ÎwÈ?]>=Q'½2?S6zôBÅö?©Áð‹(z?Ñ8
Å4FGL J0049.4-5402¿Ù÷47r»'ÀO‹e<š»À:v©ò­1À<®Ð"¢§@Nu*¤n_@j<÷T?Á¨òÒðÓ<?Â.À‡ÅÙ?ý­X"?…@n>§Z¢c¿å3êH֎¿Ü–AöD•[¿áM¦ a4¿áVÊýiͤ¿ã±—¢H"Ä¿ïÿæ4|ßOAGNbcu3FGL J0049.4-5401PMN J0049-5402?ï Èñnìn?{³'ÜBë?f""í1ˆó?c†Ý-Â¥?'(ºèø'?wíö®ðt"?ï`{Ljso?"2CWPž¤?V¥€M>h?gqÃ÷ò"?'†/
!^N?'Àþ$c$ð?î)`€qM?ŽE]ìk¥?€\¸×°{±?rɛùø}o?©RÅ¢Ì5?Š=Ä/2?îëéƈø?'€c>ݪG?t'ÚKñ\?a<öš²ÃU?_"ð›äØ?@±y*/í4FGL J0049.5-4150¿ìؓ¯ACÀRÑÀÁü2À;pÝF—"À<ÛÓÜí@ [k¤hՁ?þìZ{v™?ΒÉ[S7à?¬RÚ?âeIÀé>È?öÿ¶ßO±C¿ïýà5_]^?ﶴÝlØ¿ãN$ É8Ä¿áÅGMƒA¿Âh±Å4}
¿æ%µÁÃY\AGNbcu3FGL J0049.4-4149SUMSS J004938-415140?ï¨äMú?ó†š\¦k?7-
š8à?2ê]÷ê›C?…BM"Mïˆ?ŠÈ'(Æ"?ïm°I㶇?"&ÂÝÉ?QàÁ"—º?`¤†S6Qh?'+ê³õ"?'—÷@p?íù^¸7*a?öó|k±Æ?s	,ü*…p?a¦(½Ï@?®îÝ	B?a!BûÙv?îd;¼½Ë?–"
z,Ç?d²Ж5¯?bwù÷‰œï?­Ž›W*¿õ?–[ É'qy4FGL J0049.6-4500¿æ'ÆnŽÓîÀRo~=ÁÀ:ØúÕS"À<©"3(Ky@NÇÉ-@©WÚ²h?ÇlJ«õ½?®»¬¾åXŠ?㟮†¨Y@Óz›§Ó¿±V
þ'¿æ̬€üꢿç{é»â¿çk|·¸¿ïÿÿ" 5•?èiÇy¦µAGNfsrq3FGL J0050.0-4458PMN J0049-4457?ï¼WsÓDm?wàΤ¬¸ð?^lFÁh¹?Z]up­€È?zO+­o©?ugäå!?T?ï#¨AS
Þ?œ×?=LÇ×?eSéL»Q?vf®æ3,?˜àz¬Ú?™¬Ôíp…?îÓv¬7?®ÌÜß@É?ogáo?rFÔ¸‡?ª6îœàÌø?ŠVj>A×?ï.¯hÜ?"¯•I!{?lÎÇüqÑ?]fþå'ï?–EVD÷?€¨¤/ð_F4FGL J0049.7+0237¿ìöÙЍÃðÀNï
å6PÀ8íeéŠsÀ<	"¾pé@° í@P'½´+?¦\‹œ*îk?­ODœù0¿@CjÆGwŽ@þÓºÒ¤R?á' ù	kº¿á'[åY¿ã›.Y¯ž¿¿ák7†
¢¿è'Ì®š¿åÀ×@n/3AGNbll3FGL J0049.7+0237PKS 0047+023?ï¼½÷IKÌ?uãdnâʨ?AšærZ•ý?;ùÑ·nµâ?m§ÇÇ?u¤X2{Ó?ïÉÜ­G¥˜?ƒ¾1}t?2(:ÇUh?S¨^†	½?yï%¯¼nH?å†‰§|Û?ï$4
™$Ô?}}îʚ(?lœè1
¯?_FEΝJU?—õ‹ÕD:?{Gï‡ý<?ï͐oW"?bþ,k?MÿXÙX=m?A+:Öï"f?uwÝ`©.ó?`á¼Fø4FGL J0050.0-5736¿À3eÞPÞÀMÁe^(ªCÀ9¾®"½š*À<gKrÅz@k"K÷¥@äwC-|:?°ZöƛZd?f7þ…<Ñ?ÎVüfŒ@¿ü'Çðð¿ÎÑèÀsM*¿å!aña­¿éÅ%nO¿åÀ–'õ¿æQtœŠâ¿ïÿ¢AÞÇ¡AGNfsrq3FGL J0049.8-5737PKS 0047-579?ïîˊƒZ2?Y¶¸ƒÞA?5õðÌ"?-èÙcýYr?\멽D)?Wññõo?ïÝïáe»?y)æ¢/äŠ?!^M80X!?=íŽéہÂ?pò¥‹žå?x/KúD?ïL½gq'¶?{Œn¬x½9?eÔFSVÊð?YótǬsó?"­ÊGdÏ­?yåGÌ!ºk?ïðbRå·ï?K²CS°q?7¸(\O5?*^ûJ´?YMP|d?Hö*i¹–Œ4FGL J0050.4-0452¿ïÞøڂÿÀPð¼£À9 ܝ$h•À<cæYeÍ@"Eò¨@¯ÁÄ[D?«¿ gå©?±·ðq@­¶åû7@R҄ǥq¿Ïá
?x¿âýW^‹¦'¿æOµë÷ö¿áï åRÖ¿ì—tË"¾¿ä¡Z=c7ÞAGNfsrq3FGL J0050.4-0449PKS 0047-051?ïŖa€¶?píN)s/þ?E‡…ñ\c?;7ÁL:?zƒînæÓ«?pBÓœ¢«?ïׅ™É#Ã?yƒþÇQ&?(½bS¹&€?C
Aâ+Ù?swHÐUN?xˆµ×>Xõ?ï@ŠÁÒ?"ŽLì.£?sԔù+á*?m>êø70?˜XÒ°\Í?cQ1:?ïèñÓq?T\îRxRÝ?6[ãAOÊ?,ÓĖŸ˜›?dB°ynz·?R±Ï(¹t4FGL J0050.7-0929¿ïlÝúØ´ôÀRSÞ¤e¥À8Q'M›À;\ΌÀmC@Q(ÜC?þ¼~ ïÏ0?œ‰8DâT–?¯Ið !Ú,@§¾öJu@?¤T¿?"Ç9¬L­¿×£I›ªjø¿àø%
{"¿ßÛ¿PãG¿âiTWp)^¿åP}'%VÒAGNBLL3FGL J0050.6-0929PKS 0048-09?ïŚÊÆ9•?päKN1Cq?2t]Ÿ¨nÿ?(ÙPyCÐ?|TÂè­U?p¶	,Ç?ï¯Ê¼V-Ö?Œ´¯íRv ?=F1š?¡L?QCL'$A?ƒ#]¢Œ?ŒÎe²ü´?îÜæôÕ?'QÜ;?}—o4'Â?x†dïl-?'qÝÀ?ŽYÍÃ9"?ïd™"#È?€{öÌ#Îÿ?E¸¨l=€Ó?9ºˆ3ØÓ?'¿yšú?€eÍĸö;4FGL J0051.1-0648¿ïm†½b»PÀQk˜ñÓíRÀ9r}7%À<©&¤¯@€|ªEä@ÜIwBV½?±üàeÛÑø?ÃïÙÂ(¯@ÔçhY…­@Sš±ÇŽ?ïøÇǪN¿á½KÙÅÚ¿ä>Ðñ¼¿ç]žk»¿åv"@Áç¿ïún×S9AGNfsrq3FGL J0051.0-0649PKS 0048-071?ïÎÇoÖI?q$Ó,ô0?X쬈²?U"gÑåí¨?rœDµé¹3?k×ç}4¶?ïÅæòôk?ƒÊº%Žñ?>½&Ó^?et"ØüÕ?{ [#˜š"?€þ1níôD?îÆ;p€9;?å¶4ݹû?'ûÑ#ÒV?€}Ì?ÈF;?»‡fïg?Š¨®ä	—	?ݳ™?q'ö)Žc?P'au¹?B ¹ oœ?†Ð¶zæë1?p¹3'!áÅ4FGL J0051.2-6242?ÉïfˆRÒéÀK6W}•WÀ8¨ìëPE"À;š‡–ü@ÉI®áÂ?ùWêï̓?§ߜ]?¸'\»Aßô@¢:lãX*@hη	?ï1Çù(uj?Ðó=å=ÜÚ¿ÔæФGÈl¿Ók={5«^¿ÛýÕî´~!¿Ý̩܇ÕÍAGNbll3FGL J0051.2-62411RXS J005117.7-624154?ïæœ:(¬?`¯Pæë
?7ø#˜N8?3ŽÒ—Fö?fdÂòàv?_A'6?ï¿rzÄ?ð*5¢ƒ?4ï
ÌëL-?MžÅªB~?0Vsèÿ?~¬m 2?îl=$ýÌÿ?–ÏaLÎW?"µTB}^?…˳Ÿ37š?¤À[ž?'nÊ?ïx¿'+ª+?}5I컺Ã?D2KzˆS?;SPr_£?GV(.æb?|éÈçޖ´4FGL J0051.5-4220?Ò'55c['ÀR²~|âÀ:Ju†"ÚÀ<vÀ5¯å@3"±¨Y%@rhż7S?ÂítAVâ?Ñô>Á0âK@	æb I@	sM힩y?çÃßoŠ¿å­çχ'0¿êRª\_|g¿îô±ë±¿ï5ç­ù¢ï¿íO›ÿO€òAGNfsrqPKS 0048-427?ï5Nê»%?˜]֑ûÅ?}÷"Ê	Ý
?|'ž'4×?'ØK&$*?"óÚý¼k?îN"‰´?¯*Ž(tˆâ?ƒ™"_·–œ?'iWS~@?¦0©É?ª5lü˜P?ì({þg ?£†bH»Í?¤aæ1ABÖ?"ÖIÝߊ?´‹,öd!¥?œ{õ\g?îè7ÚI?"Nâ6$ˆ¸?†ÑÙ?ºÙB?v'ÑIéU?—…,g¯JD?~ï›Þ<«4FGL J0052.9-6644?Ý)4Á¤÷ÀI28ÅCÀ;DʈNî{À<ô±v/@žë‹©ÁÛ@m‹Ù½v?ĹÚVÎû¿RqÔ®˜"?‹,1"Å«@d3¹jð¿ã_mži3¿Ù(À]ӚǿæøÀ$óª¿ÎïA–Î82¿â ³Ô®Bž¿ÛÖò FAGNbcuPMN J0052-6641?ïÐ1üÖ?pº7fŽ5ž?7ÖÆÇë?/µ}¸ˆC?v‹º•(‹?p-©pÔü"?Òu²?‹ËUñÉg?9c¥­6ø?NKðùí?ŒŽ•n5)Ó?Š²sDÂñ?îI­âZxˆ?Œ³I8ð¶-?qIáé̄¡?dG=Ö9—?©;åæå?ŠÁ4¤›Óz?ïŒÕ|µ?r'dGAq?Uê=Ñ«$?F°&.X´³?Š>Bþ«p?q¤['sé?4FGL J0054.4+8627¿ì«b%Rä˜@7"æŸê%À:ŒAÂB/À<zxQJ@Gœ£º.å@Vº «q?Âàßÿ.žÏ?¾Þ"4³;?ô׿T>E¶@'õf?íâc¢fǵ¿äê>xâ¿ç]?`¾à¿ìiD#‰¿ïÿýaw?ïÿéÅ+ÜAGNbcuWN B0046.2+8611?ïCmûâd?ª#-ØûÝ?mÑցܼ®?•$R@ǍJ?:®à7Ý?ŸWFł7À?í'gì&i?¯QL"ç*?Ð®Ç‰˜Ð?˜ln
pΔ?¯q7xÍ?§g ˜	Ú?îDÔ»ˆço?ò灃üñ?'¥¹ùH?vÄBɋúÉ?§	EÉ*Ì?Œ²ÖÈN‡?í2óvÂ?™­ûx™Õ?šQQjAˆ?ˆXÓ$Ž&Ê?¯ÝÞ½c?"ýé¹®4FGL J0054.7-2455¿ê#óPÞلÀU놘5ŒÀ9igH
¶À;õ8Lw§×@ %"O…y?úîuÿ`Ð?±YéA¢?³¨Ö£eJ]@-J¡!@§
fÅÜÄ¿æi'z™#¿Ú¡5Ú­` ¿ÙWQ †¾¿Ö4;‹ú¿Ø¦•€…K"¿ÞAÒ½ý|AGNbll3FGL J0054.8-2455FRBA J0054-2455?ê8Äá¾No?Ç"´¹~?gV;`?{ò @Ѫ?ÆÀäåmT?ÆÄ]:Dƒ¾?î³arK:U?¸Èeš;oš?cLìÃ?'¥æÏ?£˜´‹i?¸VOÏô'?ìú ݋?£ÏÉÌt]ê?v¯‹èæsÆ?f܅
æÇÊ?¶Äâ…@5?£Œ%aGãµ?ìýò®(?šÐ|÷7W…?f;''«qF?Vó
ÎYgß?·e§3U38?šƒP¬z\-4FGL J0054.8-1954¿í+¶F©ÀT¯ƒÏ,ù]À;V¢¤V§À<³6z—@·"6Æf@ÛeìÃã?Ë8àä›v?²'xÛJ?çy>@Øb@q¦KÝ«?ïú;Àu{'¿áZ³À6fn¿åôIÔ_h¿ã=ˆÁÛC¿êÃ
¬+l•¿ïàbb ´AGNbcuTXS 0052-201?ïœc<ªi[?™2[Û°¾?NuVب¬?WƂ¿wõ&?†ÿÛgÛÓ?—Ðt²Ð÷H?ïv¬"OЯ?'\¹¯ª¶œ?MφŒ5÷o?_"ÄLÜà?;ña¤:›?ký
UÛ'?î–ۘ?‡´K…µÀ?lî×Xð8b?`<9µYê?¢°ž7Bø?†lúOυ?ï!Ç"a»?+SD8àæ?W/?{õܼ?K°á8«?º?šT'¼ jÃ?"H«à
4FGL J0055.1-1219?æ¢RÄYFÿÀRʯáÚ{À9ýÜ-'àBÀ<m×ΈŽ¯@¼p¬'ð@
'¤Òh?¹ãD![ß?ÀÞÏ-Ðã@F{¢7ÍÍ@2"iY
?ïç«?´Jö¿ÝA"ßþÙ¿ã—všÙ5¿åüŸù/+¿ëC0×8`š¿ïÿÒkÀAGNbcu3FGL J0055.2-1213TXS 0052-125?ïãÓz̞{?^Ä:â'æÕ?J`8³Á?Bkþ
ZeZ?e"w "'?ZoG2o(?ïÊð/&û?'¬7ÕóÌ?2Š$H¶Í¿?R*Ópч©?y_F;an?Î%,B>?îÝᗊro?Š3Å0Hü¬?šþ}åIL?zÀê(?›vMÏ¿
i?þsèl-a?ïÎö¼*?bvý¢HF?Q©ÓüÐY?C3ßá0Û*?t?¼¢·ã?`֑õ"¢4FGL J0056.3-0935?Ò0WjcåÇÀR¸ºÇËÀ9}îþOü˜À<÷FóÚX@ù¹î"ÝÑ?ýÑ–^{¶?°_˜kòˆ?|OðŸ%?ÏÝ=ëô@÷ü\‡jm¿ë' À¿Î7¿ÓƼgyâ¿àÔÀ·Ô£¿Ú:@m®YD¿ây…'`lý¿£\»~óAGNbll3FGL J0056.3-0935TXS 0053-098?ïãêfä?l6U'"$?+@Ÿ("?+ii;N9?jd82i»?jÙvçÿi÷?ïË=,V4?£ÄÔGd'?#{øó…tú?7÷¥ÏõÊ`?yŊ
I͇?Lï¾w¯?ïPY†Ö?"nmžô¥?g¾!¹>R?Y+EÓÁ|‰?œÞ0ª·ýd?ƒz·P~q	?ïfyã-@¼?x†·rÑȘ?I@Õþí]‰?;;?'f¼ê`}Œ?wÍY:Vp4FGL J0056.4-2118¿çñKJ'[žÀUþ!ÙnœÀ9Œ Á@§À;ý˜K$Â@"żãÊ?û·ü«·©O?³+»Æû}?¿›?¡€˜Â@Œ˜¼úDz@	Ê'§…?ïÒ"4ÕË¿Á9‡ ÄÌ¿Û<á²·ù¿ÕŒò3Ž£¿áV:¿n•_¿ìcxt…äAGNbll3FGL J0056.3-2116PMN J0056-2117?ï±&ãp¢"?'ÿ¦7?ea€Ô­g?x÷Åñ8?|»ÍÝ«_¼?…êî³å)?î¾A¶ç?³%é(xðN?k!ÇÐ=g?‹à‡¿¼§?¢iÓ1¤Šú?±îÏNù?î?æµ3'?'t_go?M¤«hô2?ˆ£ý©xm?Ÿq0Ó¥ñ?‰L]ÜvÃ?íL	¾C±•?œÝ´Å¾?s
"gcá"?d‹xêa,û?´nØ×l56?œž@AÇ4FGL J0056.5-3936¿ïÝ?¶¤AhÀS^/@_k À<6ë!LÀ=¬Âý@2@½}9;¶@%1ÛD^Õ?ܪâ`?ï«W½V@)x]@°Ac¢'»¿ïûvÞ®¡"?ïÿ™=SG¦¿ÄOF,Š¿ãuC
›Éö¿ïÿ¾AÏ?Øх™1"ÎAGNbcuNVSS J005620-394144?ëfg·0=?¿œÑÂïW?¹-ó#d2x?¹#Ð2w?§=žF3Ét?¬¥ê´º+5?èÄÌË.VO?ËJ´Ã´N¥?¾¡ºE¯B?ÄòÂ-òþ?»7ß`Þw?ºÌqEl«?äþÏûëe"?°‹¦±VÊY?œh¥°Âx?¨<íÎæ3?ÆqWj¡§y?¦ÃçIjî?é>qñD?µ-¼HªÞ?¡:Oa*#?²óL~á?°Í‡Ñ´Ñ?¦àaE‰4FGL J0056.6-4452¿¹ÂN<РÀRg ù	lÀ;/­¯ÑƒÀ<ÆuŽøUè@ˆfed³´@½ãÖÕ?Н™šäó?Çj½m^R?ò‡'Ñ(| @"'R"aª?ïþ·€ŠT¿á3A
ŒJü¿á*XÎÎ.Í¿ë)«Êô…x¿ÙccGP!¿ïÿQ"W6AGNbcuPKS 0054-451?ï'LöP)±?š@gDÐÆà?hƒŽ fF?h.*4?˜ðÄ6½?™B:Ԅ "?ï&–¢!n?›Û>öÖg?cÁÂ+¸ þ?tÝJND2?˜µæDÎ?˜§Kª(þ?í=£Tü]S?–%{»2?xkñ§dµ?8w(\Ì?±ôÊ[³<:?'æ/ÎÕ?îvÎò ?ŠÐ}Gß?hÏÙfšÞ?`Ҙ†•å?§!
Êt@?ŠiÒép
Ÿ4FGL J0056.6-5317?í3[½sœ
ÀOèMüãÀ:ïiÓÀ<ÔüA.žy@õPŠ\õ?ÿÖt|?Íü´Ük%h?É-´C>??ûG
‹ýá@n³}ÆTc?î9•"zœ¿á,c5Y~!¿â²Ÿúܪ¿Þts®M†¿æ̚wåê«¿ïûç6Û^`AGNbcuCRATES J005630.93-531931.5?ïí+›§(?`¶t"?:‹ˆ?7mY˔p?_xè¥ìÏÇ?\_vJË"?ïÄĆNU?S:r¼¿?*YwÅÈi'?AAzBYœ?|Êñ§=
?€Ó$"NÔW?îØ3O=P?"`u¡B¿?q©\£©±â?kÜõf½q? Há6–ôÌ?'7‡d;ô	?ï±õ~³^?gGt
Cº?L™z}à?;~#Phˆ?õêÿJ"?gQÊنª4FGL J0056.8+1626?äȱÚ$›ÀG5HUÚ'(À:úÀ%zÀ<ŽOÙ\'@Z%"ü|?ýÔ§Ý);c?×spºþI?ÍËù'ɝ˜?ó«¿¼CÎ@Ÿ''À1?ïԘ"¡¸¿è¸¸G¿ã3Ìý¿Õý-};¿õ¿êÐà"&þ¿ïþÈþ3:AGNbllTXS 0054+161?ïL¸ø ō?•§aý*s?ftæ½´ ?`"(-V?"šD8O—ð?"vóøŽ?ï,ɍ$d?"g	Ҁ.Î?P•ˆ¢`j8?WhVË<å"?™]uÑMyb?"¾K§™á?íª"	ç?•d8îƒ?ŒoOáF'X?€3|H7ç?®;2×­½&?ê—>mÓF?î]*
±þ?l7LL›T?hŒ'
~Ö?`¿&þ3â?®(4–D%?ŽÍžàk94FGL J0057.0+4101¿œ¥È»•ùÄÀ5×qûÅޜÀ;RÏè
?õÀ<Å ªšrÝ@ '¶%–h?þöêB(™|?ÎxADÃÔV?È#ýu·O?ö'/ðˆ"¸@²æ˜>%¿ìuŽŒö(¿ïþÂé<+?ïú½ÖÄ.¿çÖBL*Ñ¿Ñ;\øSŽ¿ïÿŸ‡ð#êAGNbcu87GB 005415.3+404404?ïK$'äª?˜½|ÛY?SFrÔAÁM?Q´Dêí†(?•gv#ŽŠ?˜7•p~·.?ïNïE«‹?"*°NF­?Oíb¤Zœ‹?cU]A?•"¬7'¹²?"~3ší?í{s.á¤Ç?–­Ù¹²F?|ÚßÉy˜¥?nÙB¢Œ—ã?²V¸Œ[@8?–
åî.æ~?îÌá%Ó?sZøÞ?M©¼?PîóG"?¢È	ž­°?UÃQv4FGL J0057.3+2216?ã;e¿ÞŽÀDIúÁҝÇÀ;®ÈÕÇGÀ<¥h[3,@¬ñ\y'´@G•övêB?Ђ§z,ìÈ?ˑb"së?øŽv pMp@‹ND†˜?ç{âN"8¿Ñ!Åâø³0¿ÛK·c"ä¿æ#ª"" [¿çñž¨ÍD¿ïøuÈ9pAGNbcu87GB 005452.5+220227?ïý‹_+?'4£äÔk?nf)û3é?c»jÇ;ßv?š‰T­"?)t5c±?îæUg´š?™‡#Pw[?Zt°*EÃþ?eÈÆ ÷÷ü? Çd1w?˜¼²ü*?í'}hU<ä?•S¤å±ëï?ì¢\-À?'†êy…›g?®í㫦u?.ˍ'Ç?îI
J*œ?ˆgð'Ç(c?t´—€(3z?`Ÿ°Ò«ƒÿ?¨Ø¬;XOÖ?ˆWâš;†4FGL J0057.7+3023?Ü­eqáUÀ@:2 f<uÀ:]á‰ó3iÀ<qƲ˜¬@à[À6ã@/¿üñý?ºW¬5Ów¿ù/£©	q?áájžYqá@h…2`z?ïÞßY—K¿ÚßùD¤õ˜¿ç2Ö·1Z¿â·U¼®¿å"÷¡aº¿ì\8åú›<AGNrdgNGC 315?íÆ$¸nJ?¨™$1Xí?qwdŒˆõ?c¢)'½Çc?°·i!tÏ?¨º«¿ÐI?ï#ˆáéÞ3?˜òÛ=És?QVã´'¿?_	ãG¥Ú?šyu'¨ð"?˜mñiA#?í1™h|
?—0Ú.á8J?‹¨%Rag\?y|E{ŸÓ?²þ0ÓjÚ?"txžç¦?îÍøi%ì¿?€0´µE‡f?ƒ£ð©P	?lG`ÿ0s?œoeâíÀX?{P¶ÂŸ÷4FGL J0058.0-0539¿ÆÉ'?f{ÀQ1&éyÀ9àL'ÿzÀ<>$ìz@Ž¶çˆ:@Œ_|gY«?µ¹f"‡Ý?š%™¼Úç?å·;"@ßÅÍÕ¿¼o¿*¢Àà¿äu0cu^¿çéâ‡I5¿àïâEÚÕ¤¿ð?ïÿÿ" 5•AGNfsrq3FGL J0057.9-0542PKS 0055-059?ïîÓ¨¬Ëƒ?U¥³ü0?<~/LôPÑ?2£ü!'u¾?[9"Ó+ç_?SV O&4Þ?ïÍiŒíÔ¬?€.ÐDdç?+4ìÊã;?I7Û!äò?xq'(çR—?§+K.?ïIÕx>xó?yÉÇ«?nœÚ Iå?g!/^â€Û?'ñµ¤0Xƒ?uµ	kŒ~Ë?ïàÌÜ)S?\{ !<¶Ð?6›{Vʦß?-K²ÕI=¾?l_´kÓ©"?["&oaѽ4FGL J0058.0-3233?앒Ïâ>ÀU>úç'À9?ÊKM
À;ý±Ù+á@›4
MÆ\?þ§"Ô@^•?±MŸ^ï=?ÃüiÈp@ÒàýÜ9Q@Ãö9'­š?Ì♨28·¿ÚtØdZ…¿ß´© !óñ¿â—¤—#"¿å_‡dU¿ídÂw^[AGNbll3FGL J0058.0-3233PKS 0055-328?ïl'',Ms?‡ª3Ûµè?pJßa ±?l,'Kè"?Œ¶"\J˜?"¡].N?ïgE
ŽÁe?žÎÉp}£?\ƒ—ÉB÷?~«é4€©?'O%<‹??›Ü,ùjõp?í¡&œO½? hénÁsÌ?¡i-YTv?–Æ…v-æ?¤"'
µ/È?"ªHϳé?ï0mÿéÖ²?Ÿøӊ¥?b¯®ëF%?SSFÒIr~?—œJ%aàê?~pƒd†Ïµ4FGL J0058.3+1723?í‰ëÀÀF¹àÞ҈ÎÀ;ײˆä@À<àòŠÌw<@"\øžC"?ö¬ôI:Ü?ÙWM¤xšÆ?ҏ4¹¿ª?ûG&Ɖ½@1ƒ°¤"¿ÎЈgB.¿ï¼ÚF2y?ÄO{τ7?ÛbY&D¿ÕäŒq'êS¿Ó]$É8AGNbllRX J00582+1723?ï36TtM#?"…›¯Ù?V~ûT9†=?T¨óût?˜1E¼2à ?"ìJû?ïHƒ¼êÀÌ?"{`Nœ,?M
Šë4?\âu³… ×?–4—_?'™pŸµý?ìދpȑþ?Ÿx]ô2@?~ۏíi"?qk?^,¶?·ëzäßD?ž(t|•ú3?îpÉûû'?—ù1ž÷\?Et6Nžxú?CküO.'?®£"‡Î?—æ]ýѐñ4FGL J0058.4+3315?ßóTïN4ŸÀ=™-ÛÛ]‰À:ŸZ±&~À<ƒ3ÆÖé†@¬nëÆ>@iød*L?Ťò}¶d+? zƒB®êþ?Ö¤b‰·ú@M™»ÓU¿ÚWvÿÄ^¿êxbý¦3†¿Ü›aÅ¿ã½#â]¿æÖ©ZýV¿ïÿ¼ä!}(AGNfsrq3FGL J0058.3+3315MG3 J005830+3311?ïãVðoIª?ipÆ5žEš?.v?
?6£íK‡å?jÁ«Ÿõ"?g£Ä¿?ïÐ$1AC?€ä|â¬K¨?ªPƒ=•?*YýAj‰'?w›>dS?€Ä¥§f	?îî ]°–Ï?…Xy"êæH?re"ÚJ?sO´†7Â?¢H&ï‡?íaB<^?ïí ñ<¦?L+o±u?êFŒ?•ú%¨fU?a·¼"¨©?KÁ\14FGL J0058.6-1140¿èÊ5ùêšÇÀRiÂ;ySÀ;Tük 	‹À<¶g÷`N@¡'ðµµ.@Êyžø?Äqw¼zL¿£ð ¢³"ã?۝i?þÁ¶é¶'y?ï¹c<{¿ç³ì+7¿ËÑþdõM¿èõ¿Ÿ½ 	¿ÕAé"h"ú¿ßÒ=ºu²4AGNbcuNVSS J005832-114050?ï	T¤s.½?'>¥'ªŸÑ?QpCÌ=Ù[?DívÆ@àø?¾g4ÖJÁ?'
G"-?ïWOw£ù?—4¬¿‹ù?U0çl¦e.?eƒO KY?"ºçšA†?•"‹Žä¥'?í«®[dÍ?'ã,$üPÌ?y¿ý2aGÐ?k«¡á	?±Q¹Í#?'yÅŸ?íH"Êè€é?›ùtij%?`T¿3·Ì?[o‡ËG¤?µ8³¯#ó?›í«²WlQ4FGL J0059.2+0006?«žØu[þ'ÀOXn¹ªÀ:Ôf_°iÀÀ<g[±×~@ðü@\†Ô?Æ3°†›;?!ßÑa\w?•GÒ¸°Fk@Ê}ª{¿ïûSþ"Õ½?ï"'úñ¿èýk@íù¿Üo<"ððÿàÄŠ]¼t¿ïÿ·¼]êAGNfsrq3FGL J0059.6+0003PKS 0056-00?ïàHM½Ÿ"?hK#B*cÉ?A
™÷ã?;§€{I–&?kp/›âs?f‰7oW?ïÍW½?}¾ƒ/Ÿ?%aÎsM#Ó?8"z̦O6?xÉÅËÞ8j?}Ž"?íÛãÂú<?"*Öö<€F?€v&K3í?q¹1Q]Y?®$>Q
Ï5?'atþl5?ï*®œo??rI(°?S×@=…ä@?F'‰Ùá8)?Š:lQ3s"?qCUú›Ö54FGL J0059.3-0152¿Ôÿ§aû•ÀP+±mÀ: ö|ÉÀ<om"BJ'@!1‹¾9·?úJ"H)d}?ÉT™_b@?À:îéWG?öäŒ×ê7@w¤!¸?ïNëUN.¿Úb/ »è¿ëM&ßgÚ?Ù>&@Üi"¿Þ‡j'̔¿âqÐý³õeAGNbll3FGL J0059.2-0152RX J0059.3-0150?í‹(hPû\?«ý1¼k?]RÔø¿Ú´?SÑhÙ?³1qi•%¹?«ÁV·¬E‡?¶—U·?'N·¦y#—?Fè FóF?V÷Á3Jš'?ŠæPU»]ç?Ÿîö?ìØ
~Çå‡?Ÿ¹áߋ?x	Ù&9?fºѾé?·¾CyƒAd?žÎÉE2°ø?íFÕuøõ? ×·ë!Áî?sÏX³h²½?p§2,i{Ž?´Œ^Ëù­(? {¹èû(4FGL J0059.5-3512¿åÄHwúÏÀTnñVIÀ;-‡˜æsÀ<×hL´@ '¡R Œ?øàLÜQ¥?ÔÓ)=+Ç?Ú·æ@'?®@ºQÎ_@'.¦[žâ?Þ÷~°4;¿äRKý."h¿Çáä÷eý‹¿ÕÝmCzS-¿à_'¡Û\ˆ¿ïüjÿÓ4pAGNbll1RXS J005932.3-351049?ïn_œY…e?ƒ®ÞІŒ*?p&Öñnï?gš
oƒ?ŒTÉþ%ï?2I Ãtê?ï.{
n
Ú?›±:}ùŸ?\USO¢?k "ž+Ý?˜pXý	J²?™ Ðzn^_?í'¶Š-¾?—n¡Hí£?ŠØˆŽ@‡¿?|‡ÓÓìw"?°"99æ?"Ø逝
\?íÒoRÑÅg?'|'óM'?aÝ«¾?U~/E9;<?°ãŽ€|vÒ?'@ÄòJ™¤4FGL J0059.5-3338?éþ¢·œÜ<ÀTÐwpyåŸÀ:îßDž•'À<}þæ$Œ§@ÀQ>@s³{j?Ä(3e]&ø¿Jèåë‰?Å|ÔýGéÏ@8WÁÝÛ?ï€wSôsÛ¿çՊv'•¿éÈ	ïm¿å
@Zc"å¿îâæů¢¿íå¿ý±q'AGNfsrqPKS B0057-338?ï·Á¼êÄM?yW×t±ò?j`6òB|‰?f5)Â?vï|šÅ?tHÃ#"?ï'Ä@†D?'zY~Ó½å?M´/4ü@T?_×á¼í›ä?s¬ë9Y?"Àé†?î<ÿŸ§ã?aÀ¡êÖ"?~]H»äy?rÞUw9?¨sÝ\îC?Œx«G³>?ïˆó?‡@?u,J¨ÑÁ?c:‹0£©?UH'¹¯û$?ˆôwÒw?sB¦•'·4FGL J0100.3+0745?Û&™žïfLÀK…}™ˆÓÀ9À~à°¯À;¸ ؽ›×@~DzƒSÝ?úñ`åóå@?°'IïgÂ?Ãahz½¶Y@Y…ðoiD@
õöA:\ó?ïãqߖS¿¼j»_¼þù¿Ôþwštá¿Øót ¹3¿áÏû'½¿ëÝ­Å ‰AGNbll3FGL J0100.2+0745GB6 J0100+0745?ï¥qª4Ô?|"Ák³cÕ?l¥n'_¤ë?l<koþaR?~ôƗ5Ãn?uoˆ)%Í|?ï R9ž?¦#÷ô"—?gãrëõ‡I?}V(ÆÄç?šß'˜::?¥@ö÷?z?íÁµˆxN?¡*úCL ÷? wN/ًh?—>¥dáUs?£mYO®ï¶?"gæ;åIà?ìßi‡p«?¡Þù‡ùE_?(J.Lð?ogÛÀwö‹?·ÐA•Ý?¡Ò)bÁXÂ4FGL J0101.0-0059¿íû͍´UÀOáXâe,À:봙Р>À<[‹)"N@•)œ±|@mFTx'?Çö¬m±´¿"o:Æy³?¿D"Wá@àG
€Œ'?ïQSµø ¿ìŠ…à)Jý¿âÛȳb˜|¿ß㲁òÞÚ¿çï\¿Hª¿¿ïþÛ<ÒfAGNbllNVSS J010058-005547?ï5h$|ýÎ?"N¬°æF?ZˆWóE?P™+H´í?—ªuþq?"Ð[0°ôx?ïmDAX"ð?"4^jQO"?OoA¢ï~ç?iðá'A²?'[ýÇÖþ?'Ã}L)Ñ®?í¼£-[SÃ?"$[¢©À9?zíè–çF4?lÙl¯È6V?°l¶í?'çšn%?íï?ÏG	,?'Usͨ"ì?d>KÌÀŸ?QgÊ£5÷ñ?¯ÈNÃlÅ?'9ˆéô­"4FGL J0101.7-5455¿Ñ5G×Ò\ÀOÅ?9ѳÀ;»¸¤÷›­À<ùÓ5@"CS/ÒÖ|?öÔxwàâ.?×?=ba(?Ér0‰Š­Ã?õ©óƒðºé?ùÎ
"Ñ¿ïì'œ<Œ?ïûÌ>²mP¿ä#%  ?͗J	
šÈ¿âê¦gv¿±X•~̺AGNbcuMRSS 151-121576?ï«¢ÔÞÚh?@¿ ۊ?AÙdê·ÃF?9¸÷TàCƒ?ƒù´yé®?~™¯È@ß/?ïw¬þûÒ?'‹tÍ[íw?MÈxlòÄ?`ËZ'hýî?;ܸõ?¤/˜?íô
¨iZ_?'&M†Û×P?wÓòL®Ò?lï~×µm?­Ä×/ç"N?'@]&‹A?íqKP«Àh? 0™º†Ê0?o_,ÌáÛ/?hP{1–ø ?³z¬:íß? 6u%›Y4FGL J0101.8-7543?ì^ˆ!³?CÀD°p~]À:øóºw_³À<drû ï@ú}µ'@'°¤xí?Æ0A¦¾p>¿©cKn?ÞÂ
y?ý$2³=Û¿è,ÊRŸ	¿ä œiàn¿êÙCӔg¿ç"\¾që*¿ïôL¾´ ?ïÀÃþ¬CAGNfsrqPKS 0101-76?ïéè%ÿ?b†Ïln B?O¶Ù&5ý?P0É
x?\¯YWn¨‹?]æ¾ÑT?îێ†3?Ÿâa&Çi?hÅ'ûLl?wÃA8Æ? ºÅïd?šúûúÃ?íÜØ»TÔ¦?'wñ!ö–k?ƒf
7O¦?u:n÷bÛ?­XðüÞô½?Hµ°¢¾¬?ï&З&•?‡ úL×˱?iïb›Ë=Ç?aÓ¼
ÙË?—èdzöæ?†4T"ÿ¡4FGL J0102.0+1639?⎯;}ÀGRv‰ÊÀ;IÍ©kŸÀ<–=u¬T‡@' 'àð@P'Û_6Ç?җýãA?ÊY ãOp?óñIÈ î@ÛR¼ev|?î¥k¼½¿é"c!7ˆ-¿×»d$lÆӿ代yí+è¿ÚÒ¶Ù ¿ðAGNbcuTXS 0059+163?ïkî'¶¦?‡Ö"ÊHü^?\Äc£ü¢?Q¤ÄZÚ/î?µôëÎë^?†óØOîlã?ï(?'Ÿz?"`»ì[ãH?RL¾ÕÛ?aáþȸ)$?™ÓR
¢S?"Aoa€m"?í¬ôB'b?'~MŽ³:#?…UUµùº?u»yqô7¸?¯ëf‰[s?F(':1?î§t}±å?ƒÁ^r#~"?X~2ês¾u?LikS¸ß?¤Äƍ›Ó¾?ƒ¥Zeúw 4FGL J0102.4+4214?ë gã¨À4–™Øƒº4À9°²2í"À<Nõw/@îȎ¤ž@û–¼o‡w?´æ&eŠ@?ÃÒr¾Žpœ@'3cښì@¨§óúc3?ìPSà뾿å¸Â>SwÌ¿êiˆ†a¿èÏ{5U¿ç'kë
¥u¿ï÷§pò±AGNfsrq3FGL J0102.3+4217GB6 J0102+4214?ïö¼½hôÁ?Iâ¨f&²?=îƒÜö|ã?7í:Ï&?FÈm±»‹?CˆÔy(Ì?ïÓT¢Ç_?z¯$Q?2ÉRW,=?Q¨([€bã?u)Ö©Œª?yúã4>;Y?ï.Z}?'¼
—|†©?s0è7ðÃ?ið¥%ä¢û?˜mú¢bÎà?€b5ÌWq?ïâŠïKæL?U‹gáê×®?SXjSžŽ^?Ccç²óæŠ?cÈۊJmÑ?P†‰—RÜC4FGL J0102.4+0942¿Ê¶¿$·WÀJˆÝ½µØ•À:áüëx‰À<i
fL@ Ά5•8?ûþ·Ë³È?ÒO)~(¤å?Âå+é<ïõ?íúö -G@ãñ@J¿ïêÜ0?ï>ž¡@¿êáz~vR˜¿ºÍ¹†ÉÞ0¿çł Ù©Õ?vCA"jïsAGNbll3FGL J0102.1+09432MASS J01021713+0944098?ï{ûêÒgp?‡†ZÒâ1N?=ä÷²R$m?7>Ù}àF ?îÆéɕ?‡QÎ3‡¶à?ïšÄôs«~?†Õg¾%Ø?<ïôÁ¡i?L+ͯìZu?ˆgC=¸?†
¯Îö}?íÂ."A…?"bs›.?r.²¡ó5?^¬Ž…ûݍ?°Ë£bÉ´U?"'˜Þ¾t¤?îZaKkd?pýúQþ`?cLÄršÄg?[³dŽ*4:?©% ý?=üƒf«y4FGL J0102.6-5639¿ÉÕRWeÂ}ÀN3ք³žÀ;¹¯¹–À<¥}xÑ¢õ@ 9†˜*?ÿ›øԒ"ì?ËÞs'êÕ¡?¾Üö êAŽ?îÞx@ƒ}Î@˜ªøè?îÄ8ÿzôé¿ã×ÓÐw¿Þ'•ðŠ¿äþ£%3–¿Ù߈'3™‹¿æ›Ãu56CAGNbcuPKS 0100-568?ï~áhß?'o©ë†•?Uì=îÑq}?X>Ÿƒ³m#?žq_ïÍ?'q
_ –?ïvçìdõå?'01]]Ç?I½)sI?X¯ÄùBÈ?U⪜?Š}Iª?íéa–u(?ö-GÕ`7?smª[pÔ¨?a}*«õ
?®ü9Ë*'Û?ÛWRp?îE³®@,?'™C"‰þ°?as©±ìì?V"ÊE´±?®´kê€Þo?'Åï°ìp¨4FGL J0102.7-2001?ãòR<ÊÀTœWS£ìÀ;öÚó=À<ë…à1@"m.B]ž?ìHBŽðÉ+?è?àáVÈ?åÁ=¢wä"@¹`ß=è™@f±?R¦@?ìü辚Úâ?ïšÜ?0—x?® Æßwõ/?€3
.ÍÙù?Ɵ­¯Ñƒ¿äè/(âwYAGNbcuPMN J0102-2001?ï!€¹‡?˜.l
|Ç3?|À&wio?zHk
?"¯Kß1C?•ÆÐQ·?ïw¯Ë[º®?"ñtsf¨?XÑA·Ùµv?|1˜ wx¡?Žùäò?'ºÉÛIÙ?ìßQB3c`?›Ê%X{®?Ñx?š1žm?µ$cêêâ?™8`bQ˜)?îØ#—[q;?"¶è¯Yå?(#žT‡?8»ÉŸ<·Ê?¢e¢ëôØÕ?"½ýîÙ¥4FGL J0102.8+5824?ÔÕ$qpÒóÀ·ê¢ ©XÀ7Ü.u^PîÀ;GŽd²1@@6†@¾‰Þ:³Z?—?úØÍ?°©G¢'@4XÍ!@ÅéôZ/¿¾ÖK¦œŒ¿Þóc9‹<	¿ä->\\!i¿äpˆÿ¢´¿årðR
¿è(ê¿üÚ²AGNfsrq3FGL J0102.8+5825TXS 0059+581?î%fu<È?ªõ¿"Bé?Wü¸J•?Rg[ÖJÈ ?¬ñXÆwÁ,?ª¿4Úú?îÓJ™Ì(?¸-ÅX3	†?AЃD@?a'´À)°?®®"Vøo?¸%¹ÊjZÝ?î:µ'£†?˜?3H}ý?…¬ÎŸ4?}6@
ýù?¦ésT(M?"÷jq)?ïïé¯ã°?O*½"b"?õ›6U³á?Á&…ì?^^hìÓD&?NFÃH­ôF4FGL J0103.1+4954?æ)³»¦+À)ÖV%¦'¶À:o¬)ÜrÀ<
(¼·«Ó@M"àú+@Ä>š4?ÆíG@±K?¶zPÑæ?ìàÛwŠ{@×o?t¿Î£ –x|é¿äœG(³}p¿é½Ê›š$Ú¿æö#l¿êCá9Ñ]¿ïþ{€©Þ‹AGNbcuGB6 J0103+4959?îwžâÈK?Ÿ
ñ"[œ©?Šl0(Xµ?'ø3Ûÿ?¡ëÝ©e?š¢À?eŸ?íÄÊ¢7s±?±òÝ"-`?k0Ô¡Ôr?{*®#`"?±$I5¾ï?±mßbêö¼?ëS.]ÌQ?£ìƒì†2²?˜Lö¥_?…T!h9þ'?¿SRCд?¡'Óqæ?íHW=S.?'ÍeC7™-?Šöfôqœ'?t/•÷ÎCï?²^y6ØÛ?'훲‡Så4FGL J0103.5+1526?ywÇÁ°ôÀG«ò<ÈÞÀ:ëCø}T¿À<^1
¿@å´ã¡ûh@ʘÅ^C'?Äé)yËóß?œQö†žY?ÕõèúÕÉ¡?õ­:mº¾¿ïûœÞÈwÓ?ïÍ$Á*'5¿åÞ¿þÞ÷¿ìÄ9ë´¡¿×ãJ<º?¼ŠC:gZAGNbllTXS 0100+151?îò³¨?˜€ð Mh‹?PŽô6‹Ò?K1F­¯? PW] =?˜2ÇÊlÅ?îÌ)Ä1?¡ |·Ø
?gî[Ìr`?€bºñ>ùY?¡À÷¦ûG?Ûí™.£€?íe팧YJ?•ô£ëՆ?Š	0¼?#ÿäÒö??±€p9Ÿ4?'ÓãÅûÁV?í½Å#rZ?•p&CM`?{y™ÿ¡›'?u6ÞØþl?°_Ø6êS€?•݅Êä4FGL J0103.5+5337?ãm!Zå÷
À"gòä¼®À9¼ñÈ.Ø[À<!ƒÞFr@ y:æ/õ;?ú	»…|¬#?µ÷ÝòŽþ5?½³ÃçJý@ƒZ'ó@Þ¿¾qj¿ð?ð?عÚÂ-âf¿Ø("C2¶¿Ü¾ƒžZž‡¿Ú(ÔɎÕAGNbll3FGL J0103.4+5336RX J0103.3+5337?ï†iÔæɝ?¨©ÄL®?Pmpµ¥Ž?je«Ÿ¸/?ŒWé86ãê?§˜â§?ï[…?¤»
ÃFZ?=9J	ìœÛ?Qq)_^ƒR?œÿ¸7œà?¤žÞ¸TBÚ?íb¯8õ¯÷?˜o—á@?yaÆRtJ?p+®KÙÌ?³Tt;íY?—û½bõcb?ï(ôh"º[?ƒªŠm?a!A	?W
YU2ˆ°?˜½Jʇ'ª?'nÀ¨Í4FGL J0103.8+1321¿ÕîÄz)"ÀH³ïàÎ'À: ù™´qŒÀ<‡ú'+6@ùOH<¯´?þê»m(ø?ËBq¿ŠïÞ?»šÚ¡Ì˜õ?ðÖáù"»¼@³!€nÅ¿Ù"K"bа¿ÓŒIåQS¿à*;½ÆI¦¿ØrÁžEzÞ¿åSUèiáE¿âæqqAGNbll3FGL J0103.7+1323NVSS J010345+132346?ïÌU­cƒ?l:¼Y@å?*&dR©3?É júä¾?yöT¸õ—?kâ¾ÛJ?ïÅçLº·µ?~ÈÐs–Eª?ÖD|ü"?3Ìéàê§?|Œÿ¥'1w?~7|¢ss?îî^•±ì?…ˆ
l>?c¹¬½Í‰?YƒÛY?Ÿ¼÷ȸH¸?"\ÉbÝɞ?ï°"rßÍ?cðy$ŽäÂ?4(‡ª£Y=?!®¤CµÐØ?ƒ[¥òò8?c¶¿yÜÖø4FGL J0104.8-2416?秮%¨í0ÀUv<òϕÕÀ9î
^u×À<|ŒbyqÜ@HÇ nM@>Vð†?·‰áÚiÝ?º!²¾iîÂ?ûúÊ8Ö@ Î|O[Þ?æÇ¢u‹G¿ã¬ ‡t~¿èÉ—ïun¿é£J‡ãŽ°¿äæZb!2U¿ïÿÕ7ÕYcAGNfsrq3FGL J0105.1-2415PKS 0102-245?ïô!5Lä?W={xϜž?+³:Q'
?*÷3‰°ñ]?TG.À¤Ì?Uî…JÉo?ﻫ»âq<?‰ HÌë
?2¡]°ý?P8ÿèp£?€€v(ø?ˆd,›Út?ï-R½UÔí?‡ÔØ6°?grÝßЁ'?_ڗÎS¢?—gL™KRX?‡
ízsmo?ï•ú
?KéØÎ{Ù?8_Ğà§?0[¦4_Eë?\¾Ã¬‡îæ?I5ˍ…¾â4FGL J0105.1+3929?!t€À7Lq²•êÀ9åق½µÀ<m›2öÍ@ó	WA°O@ß^Ö?¶2«M÷?´ëÿ—û3è?üÅ,ÅZé@‹&NÉ;É?éRøàÑçi¿æÈ8–¿ã:âŠú¿âŒ™ÖÖ;¿ìæÍߜ]C¿ÜC!þ,–6AGNbll3FGL J0105.3+3928GB6 J0105+3928?ïÜ×u0?e¬É<>öÕ?AÀÒÿ…Å?6CŒã2?nä7ºÊìG?dhsÀ)´?ïÏW¬u??|\ª'x>?1-uC/®?LÑK›ö˔?w_üՒe|?zéq¤¾=?îôˆêÂ. ?‹&*¤ÝïE?'VQ
? £ÞvV?˜C¢ÿ-6ý?€8ÅX8«û?ïÛõ2Å#??WïÎ{a ²?OÿwZ+c¤?=÷\ºY!?l
ïdQé¹?T°Ò}¨U4FGL J0106.9-4832?éà:ÓÄwÀQsWæpãÀ;råx+‹À<îã>ÿP@+Ç¸æ¼@±¦»ÁÎ?ÉW_ã?ó¿³ÍØ®?ã,Àþ7~@¼È}‡À(¿ë­AJÅ¿èpúß.Ï ¿Úò yI¿àIÏâ€é¿ïÿ¶.$Öy?ïü¯ž=Ã/AGNbcuPMN J0106-4831?ïÈ_ju?"e<ÜÕ60?eå»Yo×?‹#òðóè%?pÝmRëÉ?>¯¿[?ï…òI.k?]d ×X?HOÅ´"˜"?Z\'[ë?ŒþqY5۔?¸Ê‰(®Û?íÙ+hæ‡?"ãÈÆ?ªa?a0LGÖ?"á¾à‡e?«½^…‹?Ž¸‰kºî?ï²èˆ"?r…q(?I‹‰¨w²æ?CvìKxdæ?ã–{V|®?r	"gˆHu4FGL J0107.3-1210?ëM2éqÎÀR¦JŒL˜À:ºœiànÀ<ŽO'…€@ãg_ƒH@8>ž¡?ß­¯Ñƒ?¶ÊÿB?ë}?ó>~:˜'B@F
ú"†4?×·IbŸ‡o¿ß@zC'ý¿ç*
Osۚ¿á}¸èi¿ëÆÏ\Ê¿º¥@v'AGNbcu3FGL J0107.0-1208PMN J0107-1211?ï1¯'¶b?ŠÂùRø€F?h•èØè?^"(r~î›?–»iŽÎ?‰ɵp˜?ï—ÕZ§"$?‰¹àˆ¾?Bð&Oìö»?RǶSüo?ˆÛ¦ñg‰?ˆ‡5‰š5?îË éGï?‡ óنy?sE¢~ñ?lÁໄ? Þ•Pw1*?"6¦öd©&?ïgú![ =?s̵¸?aä4Or}–?MÔSÍ|+?Ä5J­¨y?smm˜·4FGL J0107.4+0334?Ô<Ôÿm«LÀM‡æÕw–À:ˇõ,ggÀ<_"žy_@½$x°?ù@chºÔ|Ä?Äs¨è茿¬/ñ¤|O?â³Jå×_Î@Rú_W(†?ï–ÄÓG³¿â^•ýWÚ¿äæAGÈìm¿äpý÷<7¿Ös©Ïr¿ïÿò> wAGNbllPMN J0107+0333?ïßÆ
?pòÓ1¤??¢>æÚÒÐ?80D·ÕBE?lE¥•?p(¢‹×>?ïÎxϵì?êÛI?$>­8üï?='.Ž×+=?x!ÿ.`š	?~?Ä2«Û?îߕ0×¾?ˆ.V7³ï?gætÓ"~?X»<6+ Ì? ˆEªfç´?‡8(8ÏÖ5?ï—\½#ÉÖ?q˄4'?6ÉH­U?-›¬¥/¾?‰sâlÍ|â?qÌj*4FGL J0108.1-0039?î՝þz'8ÀO_ïIÏÀ:;+@ªÀÀ<}7%@'/m@§'…€Þ?Ä °¤£
?·p²o©[.?ñƒSV¿)v@Ph$»¿àd¤à¹)¿å[ÃÀ^ªZ¿è{.¿±q¿å¥ŠžT~¿ïÿªoª²Ç?¢''%ߍšAGNfsrq3FGL J0108.5-0035PKS 0105-008?ï°âo;ð?}&ô#Å¢›?g§ÚÛ¤a?gkyh¶?{»Zݶ?w)çÂ<Ê?ï=LrÑ?žQQád]e?f[yî"Ê?wÝB';Åß?™Ìç3ÓD&?šÀ0hÎ?ìH…ÊCÐb?¡Víûá¯Ò?–Ü2€ö"?…EV¨Æ_è?¸Å
ÚÿF?Tؑã5?îl×HÁx†?¼íâÄïê?+º«±œx?q¶ŽSfìb?¤çœÈük?ñêB4FGL J0108.6+0134?ïÔl+!kàÀN~ß?–À6ÉÁö¯õ&À;)׆d2¯@ìPGk#@FtÃ÷;5?†j½ýÀÏW?º²ËCàª@-ùmL3µ9@!‰q S²…¿ËÅaž€‰¿áÆ,¿Ñ'®¿åû"y™¿æPÕÛiH¿êk¹AT´¿î¤;I'*AGNfsrq3FGL J0108.7+01344C +01.02?ï¶ôV?tóÕ
7ê?[øë¤u·w?]-ghèOc?~<hgy?s3ïPÈE?î}m(@$?´£¯"¸?‰¸þyæ¤?¥G•ú,'?¡ºíݯt	?¬€³?î=ÛÏâX?T½
M_? 'Nœ¤?•"™F|jÛ?—ö]f†r?'
m ›À?J"?"ªþ3þZ?iZfÕlòY?h,œ7ˆÚª?"FÅÝß?ÔÇ$äµ±4FGL J0109.1+1815¿ïý"#–]ÀF3¬ÿiÀ9'Úa
À<8.j€@q©(ؼ@cH¿Œrj?²µ÷‹'?¯Èî_³]ª?û'{Gžû@?Ï y¿ÜÜCB	[¿á®†ü#»¿ÜÎÊ}è
E¿áäÃßt¢¿á>yî§z¿ìþ3!?•ÂAGNbll3FGL J0109.1+1816MG1 J010908+1816?í³%%†Of?°"m'Ì<Ø?vÎv{²€?mÂÒÜMÔ½?°ùïl[Ï?°Pu¼Àæ?íå9ƃm?¯×÷YäëP?wg¿Ý‡9O?"9ÃàÃ:?®¿kœÂ?­ ˆªP"Ç?ëõbÍ?? ÆÕ¢i?•/$Òù;l?‡'tüzÇ?»"´Ùo.?œï^6-Ώ?ìî"uó÷'?›yiÎ3î8?1EmËO?{Ø%þ¤?´
ôí~›?˜M²µQHa4FGL J0109.3+2401¿é©ZõÍ®ÀCUGNΚÀ;¼|óp¦À<xwiÃèø@X.8¢ˆÖ@ç¹Å‰­?Ǭ0,–¿Ÿ"|Ái
Ø?ÕZ@ÿÚÁ@‹›˜w?Û¯ç#e4ã?ãeC»¿ê$kºc=½¿Ê[ê·nkÿâ["ötf¿ïÃ;ã?ÖAGNbcuGB6 J0109+2400?îýžz1?—Š‰'W"Ï?U͝)ú@O?NÚÞ·—x?Ÿ²^é?—-±5rÎW?äc'?ƒªWߎQ'?*[>Ҝg?6yŠW²?†Ï°NÓÑj?ƒNÛª½sÎ?îf²Ù'i³?Þ]…¹V?kT'2§W?Zdw§Î«m?§ßúh*T?L–s?ï-jb:	?~ø§jb^á?TÍù][#m?FàýUӒ?™Ô)Cƒ?~·Ö¨òSà4FGL J0109.7+6133?ëJwçݟ¿ó¸SH|p"À8-Ðé'ÿqÀ;áÝÖ	Œ@"ÑéÂ&@""ãw3=?¥,È
`)?Ä=2»i"-@–6mzVÞ@hZm߬x¿ºÅM~¸î¿áœ§ê9¿ç΀2ÀG¿éokþUÛÕ¿í²˝!ä¿ïÿŲýîAGNfsrq3FGL J0109.8+6132TXS 0106+612?ïM9‹ÿ€H?'ÖW¬n¬?…êúê­ÑY?"àÜMЉ?†Æ¢r?…Í•>ˆB¬?ìPjz_kñ?Ä/§i[mŸ?f©ä
M?Š/%MI?¼Ì<'µ€"?Ãêm!Ì?ìiåÉÛª?¦7H¿3[?­'f㒾? GåbƒÇ†?¬:Hφê?™˜ƒÀ?ïLôš"?ƒb4‰"?k&Yws?b¢'£uöÔ?"<¯Á~Ë?Ü~®q+@4FGL J0110.0-4019?×5÷UXïÀS™Ì¢ÛÀ:õ"£Ö3À<­9©nù³@ ›èÔ?]?û!³Éƈ?Æ	E£ù?ÀüÆ$<k?ú÷YhQ"@¹ˆºa¿ïÿ¬=`2Æ?ïí«3õÐÒ¿Àµm ‹]¿ÜϞƒŽ?s¿èU²Ÿ$?ÑÝсèMAGNbll3FGL J0109.9-4020RBS 0158?ï⽅Rn­?d&G@kF?89ÃÊ#KÙ?4]…+á?j;B4Lé÷?c[¤9{Q'?ïºe{Ïw?"p%Òj-a?4Òež•@D?Gãou®Ø5?€Àx;?ƒÌWûEøX?îƋGJùˆ?†Å݂6?gƒõÀtj²?cD©À–ï?¢/I Ã?…™B¼»+µ?ïuLÞ)Ô?u²¼.?PñŒ"ƒ?é?D>¬T‹ž?GKq}Hø?t{ñ^OS4FGL J0110.1+6805?áàÀ­Ù©@(X¡ÅgÀ8qö_mMáÀ;¥Ý·Ö›ƒ@ %jvÁRp?ÿʘû(¸?¢6ÿ#>Ò?¶n]øû÷?à¡s†Ž$@qÓ%V{¸?ïßÑ÷®ø¦¿ßA–bØg`¿âýÝÄ쯿ݤÙÿj+¿Þ…"/_i¿ÞJ™¡|<AGNbll3FGL J0110.2+68064C +67.04?å‡Ôzû?¿'âfl¾?}8G ¾tÃ?uL䙫M?Ô}8ˆ8?¿kãÜŒ?æµUNâÂ?È ¶'!%^?…&>¦ß?–ë뙏px?Ñìl0JßE?ÇÏîòN
ž?å©'41?°äÅé©N?žÙ6ŸÛß?ŠpÀŽÊË?ÒÀô- ?¯D8'ú%?êõIH"¬?¨Ï?Ce¯?ªhÁGÓ±ó?™–bE)Â?»!W9с©?¢e`ºÏ0×4FGL J0110.2+4151?àöôAl<À4à@žUÀýÀ;¦ºq€uÜÀ<Ðà`'ˆ@"±ñ°Ü×1?úH­ž3\N?˚R¼iš?'òk—Ó›É?ʉ8x[@¦èxyä¿ïÈ8}õÏ%?ès5Â¿æi
_¹ùá¿ÅJâ&{>æ¿Ï&ż9¿Ò;lˆÌÃAGNbll6C B010709.9+413321?ï¿ùjʓ?tùŒ"{sŠ?-oÔvš~ ?&TÎj{é?þ¦åâ}?tœC™Âa¥?ï—Øë،•?AYQ[¿ù?)#]Ím9?>1-É»þ¿?‰¥7'§&?"†]Ö­?î²ß"vÈ?»foN,?f»'ŽËj?X>z҅ý?­	ÝÛÜÏ?b·I	?ï"üÃҘ8?‰5Y
è?D´Š©¡(1?B-ƶ
·?šúÃ0_ï©?‰EÞs¿\.4FGL J0110.7-1254¿ï—~à–êNÀRÄéÌ·ÔÀ:¾šþ§±À<Š®ª¢ÖY@½iLʳî@Pys‡?¼p1v´½¿–û^c@J?ÞÔâÛVþ?@9ä>-,?ïÿQ÷GË?ãÙª*áU¿æp·'¨å¿ê\Ïä¯B?µ¦ï|¥¿´Af|¶´ÝAGNbll3FGL J0110.9-12541RXS J011050.0-125455?îíA³®_ù?£vr'l=¯?\i×€W?azüöî
"? H–ýÿ'?¢ï%—÷Rp?ïmj!î¢?"ÎoEhLÔ?Q»f	ææ?c¬
Ö&?'7{#˦?"Œ"Õ߈?í<V¬.ý?•˜™¸$=Ï?ƒO`é%‹?w'†¬ÿëZ?³º ³aca?"•¢ÿƒê?î>?Îß&Ž?•¤"B.Ã5?d^˜5Lñº?c{t­Â¨µ?ªÖŽ¸È	?•'z(×ǃ4FGL J0110.9+4344?ᵊ<À2ûÕýÍö˜À:Þc'í"ÓÀ<Šj}L[ù@"'ÌñŠÇ@á߃ˆ¶?Á1¨r¥d?vëþà(è?½ªñ°±ä@Uuów0Ž¿'…ÅYïh6?ת#Õr8¿éâ6Ó¿é ž9$å?Å~{
ã3¿èŠ= ÿ:AGNbcuGB6 J0110+4345?ïwup6·N?ŒT-ø4o?]¨Y™)Òó?Z$¯X>ü?Žm˜¿,ñØ?Š£WnÐXþ?ï¿ãÀïG?'Z/ӉÀ?3L?U¢û"ÅÐB?~Ü.¹›Ö?"-÷µO©?î}
€^Š?›¾c:I¹?t"€þ6?h9Õ
>Ì@?­Ÿ83Så?šçHbҘj?ï¿_™\ž?jvx98Ï?6H¾ñd…ã?3íhð &4?
DD;hÏ?jM=m	
d4FGL J0111.4+0534?ïºB_岑ÀLxYÈÉ2À;r.´ƒ*À<À±Ù+€@ Øp±?ýñ´âg?Òص8[' ?Á8CyT?í6ͼ¶Õ@p]i!­¿îù/Lñ ?ïý°šgó¿èÆvÁþ<±?±e'«é¨P¿é.&ïX¿Ìò¦%C1AGNbll3FGL J0111.5+05351RXS J011130.5+053612?ïíw}k?Y[Uú!üŒ?0‹ó7é?2$+C8½?`w›"-Ž¾?Wª\eôom?ïË4#ôR0?~!U£9%¢?$Š¡1p2?: Šã;P?yÅ!°Í[ð?}a³QY¯!?îUH†2C?
J¸"-Í?p©…·¶Ÿ?e9툛x?¨–^fåäö?‹©è7ct?ï~ƒªû¼º?z/3œ?R	xkéz?Mn´˜à?Žæ=ƒTg?yh00w'4FGL J0111.5-2546¿ë­Û`ÀUR¾7ޓŸÀ;0÷b¢Œ‡À<¶53¾sn@C¤Ýšzj@'Ýãu†?ڊVwÜ?È žE¥Ñ‹?íÓõƒ¥@	Óf'Ò,¿í!*¢jùs¿àÈ3?Èlì¿ä^1¾éà.¿áp—AЄè¿ïü楻æË¿ïdÑ`…PâAGNbcuNVSS J011130-254531?ïÝÇö*ßý?qØ»¤†Š?<ž
Ÿÿ¥?9ò½/÷¿-?n¤H!<ÿ?q°ás˜l?ï")n:¾ã?
²`¢uø?D¤Ò-¾Rî?Wé°ØÊÝ?‰ëWNtbL?'¤Üù¦Õ?îrh¢ê(ð?'øÞØ;d%?{E?uê.T?sÚ/!Ùûj?¥pÍâ +A?'Ápão-?ïœþgn?tFáöBt?0Ÿ‰Ùڒ?0È
¥é'!?ˆs@|Uó?sõ¬¨î4FGL J0112.0-6634¿Óƒ·*à9¢ÀI6<tûT À:S@FA,ñÀ<•Ór²@ߟ²ãA®@gFÂú?¼˜ðý-½¨?¾
iõçù#?ýŸ¼ÉIŠŽ@	š"‡0áI?ϓ˜8E–¸¿è÷̊‡­ß¿æf'Ï ¼¤¿ìj`%څ¿åÁ/ÀbY¿ïöm_~ë˜AGNfsrqPKS 0110-668?ïÄPÿyts?UØ–‡;?JGÄá¤:?SͪâŸW6?zŽ
©'þ?ZëÖra?ï,tš×|? o0 ž;b?\¢Œ
Ë4à?l¬Unt?œPH«È])?žò¤cŠ~?ï
Ûâü?ˆ+_×yQ?hôö'æ?a©?ÖÎ?›…äì\>š?†ú
øUæ;?ïˆ$`
Ao?tÌôÁ?psˆ…?b&Î	›?…½X¹-€?p2Iۍ9ì4FGL J0112.1+2245¿î$¡
¸PûÀCïmÁ¤zžÀ7MØYÈÉ2À;%IfË@'P¹+@¼Ú'.?'/,¾O¢?­:­a2Ü@.&,ƒí@2od;黿"ZUû£é˜¿ÝŸâˆö´'¿á›žV—¼J¿á1xþ™x¿ãò«G£¿çåøL­W¼AGNBLL3FGL J0112.1+2245S2 0109+22?ï§US|Ó?|®¤é}?=žéG$`?90ë,Š?…=³ÖÆÙã?|(ZTƯ?ïe5´¢—¢?•l‰jn†­?Rž."‹'?nØn2-­5?'/hˆÃÓ?"£#¨Óøí?ïÿ׬O?4]ÌZW?'ejð#…H?'¸†Óko?'ÍO'dI¸?ˆ%y÷3?ïˆJ{Új?{
•ÌZ?Qîz''m?E¤§S·Kø?‹Ö'·N?z"N7¸¤¦4FGL J0112.1-0321¿ìK¤2œ+èÀPnk΅3±À:MÞÌ©'^À<YÙAOU©@sLYŸÙz@Öðd‰Ø?ÁË©â,£?ÂÞt"ýS?ýJð
­@IV‹'?훀#¦Î6¿æþ*¿æèɂ•q¿ê¯ ²¿â¦=Kºéu¿ïÿT©¥€XAGNfsrqTXS 0110-037?ï:ÿÍ?Ž0¶î}ئ?`"ãÍ'ž?Xºú½Áì(?‹xÆB÷?Œ–m­äA?ï@'ºÓö?˜Ý$©…Ô?aã{Öç­+?pÁ×µèr?•³9*ÁÃ?–}êÄà¸?îÜ°.8f"?Š1Ø:<d?p—mL›3?arÖ§$U½? "ræ4P?‡Þ+~Â`Ô?î ¿UÁ¸C?…×wZø?tÒ£ÊBáê?d 2{}À©?£Y¶*œ‰?"eĊ›à4FGL J0112.6-3158¿ïÂõù@ôÀTÓü;OagÀ;®¬A<
rÀ<õË^7ü@ m®@o±¿?ö
þ`Ï?ß]àÛÍq?ç\3rSÎ@"ìck	c@ÃüÏHýö?ê³rôb³¿ïÝHæ"ß(?ìM¤=Œ}|?¹–@bŠ~¿áÒ¨ëÎE¿ïùêqùA AGNbllRX J011232.8-320140?ï?…¿"?˜•›+\Š?s°ó
–?rt*=põ?"#V#ˆ¡?–wX¥ò]¿?î㨂êV?­IJÏ@]Õ?q'²G9«?‹7i;=šÑ?ŸAæçL?ª/"-ñ$ä?ìϓ
wÐ?œ–‹Å?D]|ˆk`?×Ä[ªŒ?µrPMdº?™¬
ÿ¡ò?í'}0|Ò?£3ƒŒ4Ä?X•"—qÇ?W»n¬í±r?³Àm€¤?£/øB›dæ4FGL J0112.8-7506?ëûäû RyÀDù}¿HÌÀ:ZíÍÎTŒÀ<'йÁWN@»Þû£yí?üž_ ÷Ç?ÅöX¡×«£?Ëë4Áӟz@@ìYZi@Þ+"ƒZ=¿Ñðh}—ÛS¿ä¡ŸAÏ-O¿à¯¤Ùš¿Ø5X§ay¿áá»;ªÐú¿ïè ÓI¾AGNbll3FGL J0112.9-75062MASS J01123146-7506179?ï"Lªm?"Ä×¢)d?{&ǵ¨NŠ?tZA…ðÓ?˜cä}HJ™?'"Ùx~.è?íÿL ªk?©TóI?{C?µ›9?Ë¯=ր?«ÈRø"?¤×7¯l¡?í	&Ø|X²?šF
 Ü?"%ہ÷9?ˆ'(ÍNÅ~?²íR[Öü¤?"B&ü)?챉5«Žv?˜
Õô²·?'–ÙY ÷m?}¾H©D?¶
ÿü[Nm?–@rC¤‹Ë4FGL J0112.8+3208¿ê^,dH:=À>ƒâCV—À83È23XóÀ;Äöƒ{á@Ü4d`§¶@<`Ÿ?u¾Ú,?±#™¸"pÃ@üm'ºZ@ÊwàŒGL¿Ö':ÛG¿áÿe:í;Ø¿åú#G,å¿å €sWæq¿êLÞÕãÌÄ¿åÄ|ÁNjAGNfsrq3FGL J0112.8+32074C +31.03?ï}†à"…?ƒŒQ!úúF?\cB.S?S3<ۊ
?*1ßµY5?'[YyèBé?ïÁ4âÊ¼?'ü˘­éÇ?5€¥VAr†?OX{ßGX$?~
"E•‹%?'d¡'C.î?ï,ë®t}é?‡
|0V‡?v,K穯'?r³¨ˆû'Ø?"×w7…×%?ƒ·é•ü»{?ïúù(·?:4ºf	Ҙ?}…~`Ào?
Ò³yÀ#«?E°j°?8•à³}ná4FGL J0113.1-3553?ïþÝpˆÿÀTß«÷jÀ9Ûà$˜e½À<'4pJ@"{ZqÍ@¯ÎÄô'7?³îހº‹¾?¶ÞGH"íˆ@^á½Ùà@Sòt|(Å¿Ï<í[¸{¿àҟt¤í‹¿ãýDcÝ*¿é oA{P¿è?b`ÈAοïÿ4Þ®÷zAGNfsrq3FGL J0113.0-3554PMN J0113-3551?ïÔ.å¼¹W?«Õ	ãqÔ? 9t€;Æ4?ãç[ÿë?ufÁ}¡vw?«Õà
ß>'?ïÖTñ kŸ?~GX®ÆØ? Mü '¯?B¦wvÁ?tS
.Ó?}"G'-Q?ï+€OþÝ?…šH
E?q´mYõ>ˆ?tÚ±u±G?–"Ú©§{?˜Ð²õ&?ïø×–æa??I{h¾Øs?Ëã…¹D?2ŽX0Ør?Iï%BÕÄô?=…ly¹i{4FGL J0113.4+4948?㓘p=kÀ)ÒŸ˜·À8Ùì©&¥À;ºÇply¦@˜ãy·|@^·E|?¦Ñ›¯ô?±™é¾·5@
jÊA¤æ@èæ5?íԗœiW²¿ÜÎQÝr¸¿ã^ö€$}Ž¿ã}FA­¿ãÕ4ûE†¿çä]­Z@¾AGNfsrq3FGL J0113.4+4948S4 0110+49?ïكJvC?d-2e³?-'šìÅÆð?#+ð¿øîM?rU4ƒ^°?cͬÈƾ?ïÜíТZ0?vç!Ÿs=½?(æ†ÂW?G:Ì쥍?pÁãxÀ.™?v"à6!]?îúGï–Ij?†­R¬ãhN?uOTxJ??jý¹­¹_?›c,ï$Qq?ƒ(öø·•v?ïí(ƒÅx¤?PÞw™»²|?!DFL½?AiFæî?aÃ7ÕÅà5?PXÉå}*4FGL J0113.7+0225¿á¡îÆpàÀMûïÝëÙÀ:h†Úz4zÀ<rû@
faÞÂC@%iF·G?ÅbB¶3¿›y¥ÂÇ»?ÑÞ`þW@@}8ém¿æó0¿ŸÛ¿åNx¾­¥?¿çœÕÃìS{¿ãR&]·Á"¿äÜ¥‡äe¿ïÿù³>†AGNbllUGC 773?ï=eŽ_‡?'6TmÏn
?`ìðö!£ñ?VðQ¼Œ>Ì?–Aµ/oÚº?'˜¹,M^?ïªÝSQ?'yV,òƒ?E¡K?dÐÄ?VÊQB–•?Ž»fÔ´ÞØ?'¨šõç£?ëÅS'#±\?¥¬Î¥oÐ?ì^ªS?yúš•Q¯?¾âã
*¼?£×¾°…Â?íëdà9×?'s.RVð?`"ï"ɕ™?P³†Ñ$ð?° 9†¯ä›?'pu+AÓx4FGL J0114.0+6418?î¼®ž'a³?ø£~éÐÀ:&xèI*À;Ëe±Ím@ ëW+5ý@)³(é-?ÅË#ÕGD¸?·£3÷(k?ìOQâJãS@=Šzº0?—p4£ý?ß&Á°¹ò¿âàKd'`˜¿×c§úÛR÷¿ç•¶ë¹÷޿׋²ü;AGNbcuGB6 J0113+6416?îQJç?£~ZŒà Ï?LϼÞ/"Ü?Hc}'ïæ;?®—¬k˜É?£YSå'i?êsî±ZT?ÆݬGVå?WÎÀgµò?v.BA·A`?Ƨ»',¡?Æ¿àÌ!JŒ?ê!µ"˯W?¦Œ¶—'?ŠþX¤3?w" «_ ·?ÅØ)ÇFÿr?¥rœÎ1n?íI¦®
­O?"|9¨lû?vÁú!ˆ?eÆ[¨o¥?´F¹¿ð}?"[+¿UÌ4FGL J0114.8+1326?îr.¸*ÀH…S`Ð$pÀ9È=ñÓÀ<"HÏ|ª@%ôx7t6@ÔQ[<f¹?§JdR:	'?eŒQ1 áâ?¿ÝϾï"x@†ª(²ý¿ÜÀêm¬¿àùL`RP¿ão·]yØ´¿Ý×}_§/"¿ã:x øóò¿á5›WߺæAGNbll3FGL J0114.8+1326GB6 J0114+1325?ïÞ2M—ãæ?Ÿ0LJk™«?-ËæyË\,?Xœév!¾ÿ?oðôe×?§t™Ìc?ïϘÁÇ{]?ÂêÚZ|?%÷ê9Ø©?Aϗe7K?wƒßÇÀ'Û?~VFgÿ˜?ï<
º}[*?€GU×3n?f
'"¥²7?c";"3ѯ?•½V¿ä®?~fÕULX?ïä8Ð óK?Wb«G9&­?6¶"$(Ó÷?'aE)ª>?hð]z‡›?UÞ΂[ #4FGL J0114.9-3400¿á^¥úrnÕÀT]§°³''À;_»QzÀ<¬zyBáý@!Á\+e‰?üÿéYËM?Á;–7¿ áŸlÂK?ßÚr\"Ô´@j¾—ÕÊ!¿Û2pžÎ¿èÕ?AßHz¿ß‰üÙ´¿â‡Ÿïôð¿Ëáw(Öc?|~Ó"Yú¦AGNbll1RXS J011501.3-340008?ï}ô§à?‰pd4ë'?@$‰²)A¤?3#…tð£N?€µ;så?‰CøÛâ,Û?ïj3Ñ­?êG†ýí—?D'*3î£?W±ÅÃ;ø ?ŽdhUÈ?)4?%؈?î#"À¦
ø?"r—DJ?fÚQ%zp?ZLë=?¬ZãG?'ÖÃ&Yk?îx‰?ˆ?•5͗G?9ª){ÿ¦?4a5ppš?¨KކE?•>†EEo4FGL J0115.1+2622¿èwBbÙOÀB~|âÀ;Êön‡À<m|ßýa@8——¶Àq@MíHû?Ô3ÿ
z¿¬¨PÁŽ€6?åü·ÁLæã@
4rIs'r¿än?Ƕ¿²]¨@•5K¿é¿¥Ò.¿ÖKIàâi¿×*Â+A¿ðAGNbcu1RXS J011451.8+262337?ïÚû6É?lHðïØ?6åøU¡ú4?03çuó‰?qlåûV?kT3g¼õÁ?ï«ô~WÛë?"PŸÄ'pø?*>½2"W?Cyq[)?"š—o;2?ƒçÇbÚëã?î¤à<ø¹?`Òß5d7?kc,3(?d
6%©"Æ?¤8þÑá?‡}ïƒö?ïnóQâ"9?y]#Ch#þ?>*}C@ˆ?3xB6¯	?'¨ëÏ>«Ý?ym²Á2d4FGL J0115.1-0129¿Í¶:'BÕ_ÀOßbb˧3À:î¯÷ªÀ<7mƒ'˜@h€•'¢)@¶';‡?¾`¿øì?¹—´<25\?ò:e;Ãûm@6ƍ?îQB‰hI¿äµ€r'¿ë)ºy
2¿ìµÀÁ¦©¿ï'›??ï;-ÇüƒAGNfsrqPKS 0112-017?ïØdqìp?v¯÷röƒ'?DŒ§\R(¬?B'IÃÒÇÓ?q<2‹ƒš?uFÃ;bZ?ïŒ_^yf¶?'uN)Š‰?Ij}™µƒ?\¨
"Xÿ?‹Q€ˆ
úh?Vh£:ò?ï–%­?"lj£&ú?n†ž*>?`y:å",?™ÜiI֚@?' ¬""´?ï°âö™ºI?lø²$³XÕ?W7~
¡?H/Nnªƒ?€ãÛiÐ*æ?k[j䛪"4FGL J0115.6+0356¿ê¹¶éûJ¨ÀM0—á2µ_À8ûá÷|þÀ;ø­•Ïà~@a$H¸@Go*ZG?¬
é½ôAÜ?²"†Òeh@X>»&²@\ìj!¿äa³'¿Ù®=•ŒÄŸ¿á1QFC±0¿à†&˜ðý¿æüÁâc¿á1´âf'AGNbll3FGL J0115.7+0356PMN J0115+0356?ï$*¸mXb?–U2•…Ðà?^¾,̦õò?Y$9b7V?™ŽÆ%Š"‡?•"ó¬Z0Z?î² ÌB?¯É¨Òö¹?wºa3eäè?iX.K"¾?¡Þ²Y5?­·@¯¶?íúLÇ?t²?œ'Iôýÿ?ˆïà^¥?|J–·"ð?«ù2P#?™<ü Ñ?í»SÄÕ?—ùØ%®f?‰bâ5ÊÜ?wŸð.ŽÛ?­òˆ±+¸?"-Ä4FGL J0115.8+2519¿à㳪M,ÀB›–À8¥´B'KÇÀ;¶Î¬ Ý[@Kn	È֞?þ¬*˅¤ð?£‹`-¸±?JïË
d?«*JX…@ãLÓi©¿Ô åΑ¿âyDÅ+áY—K
À¿ÛJÝÿz)¿Ù²†eà/¿Ý"o@ª•AGNbll3FGL J0115.8+2519RX J0115.7+2519?ïó©d 1â?X#ƒÁØJå?´_!q*?úåõe?Wyª"©?Wmݦ¹ÏÌ?ïÖ
"Œ4ý?ƒìê²ï%? [üÄðÂf?7&Ú>æÛ
?txÓ½û?'㹎.E?î¼ÿý4n)?¼K£O?gò Tl=?]瑆"Šô?¢°ß*³Öº?P£¶ªÑ+?ïôM÷nɞ?FB
AtÆ>øð
Yò>ñaØï|?WPÆ'â?FÊXêø4FGL J0116.0-1136?ïÿ£NײÀR\/ƒ{J#À9Aª>-À<?¯à,ûâ@gÈ;B¡@©½R†?©!="±l?­[Žœ•Ÿ@¢Z2{@Êæºßr?›­5F¢•…¿â"Üöæ{Ê¿æ·hí)c§¿ãY`>.8ø¿æ¿Zž\!¿ïÿZªÕ+AGNfsrq3FGL J0116.0-1134PKS 0113-118?ïôŠ›É­°?Z9þß܎?¢¹ÒV¹?»M	)‰Q?U¦ÑyB?Y[µ¹ömœ?ïßòNeò?w-‡x¯Í? 6è ûxÒ?7""ÃÌJ;?o÷Ÿ'ŠV¾?vŒ}Ý9ÏV?ï/Ò cÞG?'iéçe?p͚^Yä|?rpÐzkƒ?•ÒU[í¾?€Dz–ÁêÙ?ïû–ÿ°÷®?0Û±ŒÜç?³mÖ¿Û?

õOÖ¬"?>ÛB\Ì֒?/\Œÿ4FGL J0116.0-2745?àÊl9(ÀU ÃLŠÆÀ:ýayWÀ<Ÿ\>Å7­@!R'È>ô?ûšîcŠ	?͏t|©Ÿ?¾‰œKz§¼?ï
¾ßÏ3@" fQïýÁ̾Š?ïåt™/¿È"%Ú/5ù¿á½>!£¿¿Ø¥{úø.O¿ÔÁ*AÇöyAGNbll3FGL J0116.2-27441RXS J011555.6-274428?ï·¸û=œ?¨¡×Šc8¢?;¤R»Ñf?a°D]£ì?4Ö«R
µ?§ÄõÑÌÄÌ?ï½hì¼t#?ƒµÿQHK¤?0Fº`ï)H?H×Ù·C
?€#ŽýÛ~'?ƒ#h×»H?îuvU(?°Œ,¹ðÞ?dïö7.?Tª•š=oç?§Y›L|<œ?Œ°"Cf«?ïlJ 0úr?x¶÷j<Ú5??vI8Z½?6†u+döá?'øâÕ×Ў?xÔ"5t×4FGL J0116.2-6153¿êGyCbÖ9ÀK~r\=îxÀ:}ç&f¿À<š ]Øù+@ 3^(6Ö?üÈÈ@vÕ?»UÖ&"?´zڀƒaä?úcˆÕü÷?ýNá9–O¿ïó?']<?Ï\°¸¸Ä¿Î3BL«ª=¿áãyí+çå¿ÓQ‰_²¿âyUn"AGNbll3FGL J0116.3-6153SUMSS J011619-615343?ïF‰ ¾g?1I.CÜ}?Z‹Ó¦¸X-?U®6*¤Ï¶?•"ñ¡|­Ö?[üáxúõ?ï#ýQjLµ?—KZi ?YV"•*½M?dò°–
·?™êó©c½¬?•ó¤ý'
?íèyd‰"?ziª]/ä?~tF\'q?v¯ßä<ï?­©àëÝ8œ?Œé6…Áîø?íoË8VCÓ?"¼§8!c]?}. eø®N?pÆèíÄÁ?²®¼6îV'?"3WŠži4FGL J0116.5-2812?ä"¬2sxÀUÎÙ‡+À;Zm]ÑloÀ<šVHáñ!@õ^*Ü#@ƒlØ?Æwe'+O¿¯]ÃT¨ù´?ãüµþT.U@ÆÞþ}Ÿ?åɛ?-±¿çbz¿å"u'ÊIe¿äê•ÀF+³¿Üãa¹®b¿á~ÁqN÷µAGNbll1RXS J011637.7-281146?ï i©	ú?'¤¦Sm"?\pû¥ÔàQ?Sú™(íý~?š+»$c`	?'E¶":œ?ïi­Å¼?™²4Ý`@?KË2w÷®Ó?^köÛ2ä?'윫?˜›Ù(½Ž?íéµÒ›üñ?'ÓÅú©0E?t'í~I¨'?b» ZÁ?®Òe&vûõ?'»0¤Lª?îõî3³N9?ˆœ`aÿÀ?FÇ%Ó4¾?A1æ'GÅ? F-~I…?ˆ0Ã;î\F4FGL J0116.5-3046¿ï˜33øļÀTÙp÷¹àaÀ:üd^NiðÀ<¦ù)L)¤@»Ç{)@˜jßqë?Íåw©ïÏ?ÃD͏jk¯?ò\T)Md@ˆ|ñm@?ívѧR¿ã"Q´þ¿æ¾ç0ü!N¿ïþŸ½Êü=¿íjUéŸì?ì0…ÔÀ·AGNfsrqPKS 0113-310?ï)¯©áí?«éÈ®&ߦ?v¹–LŒçÁ?« –$!~?"XÈïA6?‡
HhüS?îh&µdM•?³î°Ka?|ÀOë?%­?"Æ1ÕÕÏ?¥åŠ¬SB?±‰[ôx'?퍖ø¬?"¼
Ù–¿?†®7¹
O×?wá:ÖG8?°Â(D&›?'¿:êUç?îÅZÖ?Öø?Œaaá)?n›\©yï¥?cœGöB؂?¡ÀœÑjñw?Šùÿa›Z4FGL J0117.5-2442¿í\ÏcÕèTÀT颣Y6À;ÁV¶JªÀ<ïCœ7Ì@!W"È×Ê­?ñøDIÛì?é!—c•?ބwžr{?ñ+k…L?ý;IÚ¿~±¿'¢Ïù'Ñ¿éôöí1Ç"¿ïí	þ±vZ?Ñh=¿çTbøóœD¿Öà¤E9¸AGNbll1RXS J011746.6-244329?î¥`±pH?¤²»"ž?iÍÔ®"bª?ex+JLÿ·?¤
žÅ^?£ªÄ‰Tj?ï\R4ó5?¡r}íÒb?V¤íöï?m'UFÒÊ?"wqz|ì? Ñ¯ˆa#?ì-~Ü"ú?£@ËeM?ŒÔ܍³®Ú?€þÌØ·"¬?ºùm´âP?¡Æq
µN'?õ\}0?žMäï¸Xq?5'øÞpcU?H¾ÔŸ7g?¥ìÀ¸{L-?žR-Å 4FGL J0117.8-2109?ïÞU¹®@ÀTa¯ž¾œˆÀ9lszKÀ;æK!JÓ@ÛBV¼¥7@¨¾e*ý?¶ú³åË z?½j°£vg@ý¾`l@½X~qJ?ïú"Àā¿×ÅÑZûú¿ås^ ò"Ü¿å锹`~¿æåªda¿ïú)âQ™PAGNfsrq3FGL J0117.8-2113PKS 0115-214?ïù&óÀ´æ?@"˜þÌqª?$
 ]â["?˜'*²6?Fa¨å³ËH?=ˆ2¶m?ïÂln‹u×?‰Cå¿Iþ?2E¡pYq?MØǧõ;?}¥n£?}"?ˆh¤³gÒh?Ð=/??Ti$[?z§áé|o?qEÌbŒg?¡'¢EÌ©?ŠÛ&<Îq?ïÑÏ'x?ræ¬á¥8?RåÞWP°]?DWrÇmo3?†.ÐkPL?qÇ>|~ß4FGL J0118.7-0848?ä¿B0ã3ÀQ¤Åm\ú­À:nÀ<~lê&3@MùÛùz@ÐÛä—Å?Ï1æÂlK®?Ò\'þw•@ùCM\ª@	Q¬«5x¿©È&ÊÅ
·¿æô¼U…ÿåë澚¨¿íb(E¿ïÿÙi"A'¿ã.<=óÖ|AGNbcuAT20G J011844-085058?ïº&³ p?ƒªÍ-–¯?Sc£í–Mo?Q&kKZÛ?~½CÊ5E?'ÔOM:?ï)cŽþD?¡x46Îy²?pUBé
/õ?"AâˆÛá?›'ÓÝ«®?ZВM?î_ÃÃè?"QZ—žI¿?ˆ¦Sîyá?zʲqp?©Àynˆ#?'£'µ+?î¯Ä' £ë?Š=tî"Ž?x}ì⸝v?fè¤Ð2S?¡óùIž­"?‰ä¯Í÷ù4FGL J0118.9-2141¿êckWÀTnð¹À89¼R+EÿÀ;ƒ|@Ã@æ-Lê@œIwB?‡B÷Bä?·dD"@;p@Ú»£@P;\Í`q¿Äy
t­¿â<i"‰G¿äÄFwÜ¿â¡fµN+¿è6;ÏÆ|¿èéQ'©"AGNfsrq3FGL J0118.8-2142PKS 0116-219?ïŠ/¢0?€5/Q'@N?Rïtj!^?Nu:¢¨@Õ?‹]Hë¯Ï?~¢;vIòè?î̲Z>ÂN?³ò¹Óè€?kàFäûä·?‡…õÉðoÖ?¡vÕíÄÄ?²˜¢¢Ì£?î¹Æå¿0G?"å[!z??Žú¹h½S~?ŠqøfÕ$è?™IƓ»M_?ŠÉùŠt?î^;8ü™?'t¢©êø?zù…õ™?n–¡¨p0=?¦Ù»Ì—É?'9 Lã4FGL J0119.0-1458?Ç'(è¶bÀS†YJôñÀ:I£–ržÀ<V>Eµì¶@ {ßaúÆÛ?úgJ&"¿??Úl'p‡R?¾ÀRëà8d?þ1Ó·¢™@ÛEPl)?ï÷Ÿnc‹¿å2GzèÔj¿Ý¾6|=é¿Ñߢ'fŸ¿Û¬ß\‰É¿âÊÕFEAGNbll3FGL J0118.9-14571RXS J011905.4-145906?î¯Rïé=?Ÿz•ªÎpH?hò¿ï'?'¯êcù&ö?£îßòz¦?™&ƒH-Ý?ïy«8¿74?'ÔfëµÏ?Kv|´YÛq?[",îüã?ÝÊì•N?'$ÈmÝ7þ?í&o²>Ùé?šñIh1Yd?{)+ú$²?hL/–O?µé›IŽf?™1Êdö!Ú?íj»ºˆ'?'q"Ö³G?fË·ùeÆ[?UuÛMØp?³óÄo؍Á?';•8m4FGL J0119.4-5354?ŽM·Ý–7ÀO[ñ•1äÀ:ÙܲÀ<µm¿öûu@×o'yÇ@Â/BêÊ?À‡‰v¶Àœ¿¨§q@˜y?è[x¦@Y
\J?ÄB§Yö–u¿éqmŒ¿äüÅd"¿¿ßD˜¶DË¿ïóO]`XZ?âM‡rO¨µAGNbcuPKS 0117-542?ïs±4þÂ?‹-ï؛®à?k´áHnã)?cX@x¡'Ê?Œ&z«¤–¶?ˆ©KòE·­?ïq!›Æ^?'XÃí¸H?S™ÒãD0^?e÷!^8
?¢B^RñF?Ä?p›»?Ÿ¥?Ž^™uqÐ?'Dæ]=k]?v7""-šu?©•DþVªÚ?‰"T°|‰?ïdVˆV?zæQFŒ1x?kKÐKwºÆ?]ëµ-ÃÒ*?»%†GÍ?xs•'˜˜44FGL J0119.6+4158¿îÑNµ«ÚÀ4"ó#x«
À;DÛ;$™<À<¥ˆI=‹@¾½º`8¥@Ÿ°ºG?Ð'L†@?È¿ˆ–'ýC?û®oÜV?þC,»–ï?ï= "Ds¿¯´Ê!¡»Q¿é6†…ÀŸ¿Ü»õy"@"¿í5Á¸œ" ¿ïÿX¥³ƒPAGNbll2MASX J01200274+4200139?î"5(ln‰?œ]ÚÈ>?ŽËZrKÍ?‰Z	\*Jì?ž×E9÷?–CÇzG?ìÀ%3#ì	?´Ã§³à?•fÆ|—"?›È¥ØÔ"è?´¥TõAyÕ?±êTQD»]?ì¶ÆFº2š?œp"¡ˆ·?—÷Mld0‡?†b~4›ú?´Kúo_?–Àï7Íó
?ç4QÏ
Õ?ª <Œà:¼?´¯EØ´Û3?žîjä/8G?È××u[?©¨–qŠÌ4FGL J0119.9+4053¿ïëá©Ó¤À5¨¡œZÀ;œqÀ6¼UÀ<ØÐÜüŹ@ ÄLˊ­?þº"Àõ(6?Ø:ú݁O÷?мXáB¥—?ú*…ʯ¼@`ô)2(q?íÜã›EkD¿±uWELå¿Ûç};?¿Òuác\ƪ¿åÙþí[c¿ïô ~$É
AGNbcuCRATES J012018+405314?Í2Ú?ƒ{\ݛp?_ϕJìØ¥?XSŒG/Þ?‰ÝÆãU®…?'!Þn^úØ?îmY&Ęì?¦‹´¨h?r½®@ª?€aóÞºî?¦Ò·Ò&I$?¥›F9Ü"?íªÛ^É+?"ÔH\γ?ˆûËvint?}p¢UaEä?¯WA9È?'¥a-²¢?ì
ª¥å?¡?˜ƒ»œ×?ƒKÿ†Kâû?vZ라Ë?½EŸ©áTw?¡%¯ˆž,4FGL J0120.4-2701?ïý(‰…-ÀT⹩çÀ8dµ—&À;YАä¿@øŠë«à?ý#8ê,Y?âWùf2å?ª²³_ؤ@ñ¡˜kœ@§é2Þúw?ïýŽ5¸H±¿ÙCSy¿Þ@áDž»¿ÚtZe&Jm¿âXQ€%TM¿Ü˜‹<3·èAGNbll3FGL J0120.4-2700PKS 0118-272?ï°ŽOë?'•mŒ¾ŒÅ?/ÙìÆ3öú?)sÛãúpc?ƒzôÅS5A?'z[E"[?j¹?µ½ïVg?q·ŕ¶n?¯%nV*¨?¢ÞWfëí³?´zâO Æ?îF8u >Z?š…aºÕS?…¤Ž¾¯a‹?"†6|'?¦3TþPAê?–-7Ï©ãb?îæÊ´³:?˜þ}Dx7?qÀ^*rAü?eBÊ[:Žr?«é‡f"?™	ûjô­4FGL J0121.7+5153¿ÛÈEÓb¬âÀ%dí0µªÀ;'³ S\žÀ<ˆ §ªÔU@"€±ˆx´ó?úï'åJr?ˆZ!´†?À"ÈVñSj?÷V%¾@Ø!ÈýŠZ¿ïÿÀ	oëJ¿ïuÞ©n#?ïÿXJ¿¼sîdL/Ù¿ç
çIOÕ*?"™N›Ÿ´AGNbcu3FGL J0121.7+51542MASS J01213367+5155520?ì¾ÔÚv—?³[ªwþãí??"è8¨Ä?6²ç	Å4$?¹éÄDŸ?³PT'Õ?ç£R(	àu?̬exÄþ?f–üàö6?…õ!)@Ç?Ќ."ò})?Ëúæê¡Lr?ëìZ7½Ð?¢ª€ÉM2?}ôÚ±ªÍW?mqŸ†ž?¾½à–öÏ#?¡²&?馞‡;é6?«">¥´ó¡?}ahx:Ó?y^š›±¥Q?ÈzzŸNŠà?«Pó3"¼4FGL J0121.8-3916?æ
"È=`ÀSyB=KÀ:¤ù8e¢À<›"´W‹@ "]8??ý"6÷
7?À—ða§dÞ?µ†
`:Ó;?öàÄn&N@qÝn°ŒÐ¿Öp¨ÿ¾Ç¿¥†K3/,¿Û¶\þˆ±•¿Ù›¨B›†¿æ'ø»h {?qs™;*AGNbll3FGL J0121.8-3917NVSS J012152-391547?﹘MÒÍ?vŒ–—Y—?Gjš¶n«?:Q­@ðÌÆ?€#C¿åê?v±SÐÜ?ï–÷Úåë?‹#ƒ÷îs?:ê 5·ª"?M‡yø"õŸ?‰jÇÔ?ŠWkáäº?îXRˆ!C?ŠÈ‹©}2?sѶ¡?a$ù'Ó½?¨Ý[u
??ˆÑ›Ž~êõ?ïùʶÏ?}v^^¶Œ?c1Õ1\ñ?Q] š…O?šº¢w­?|'nÚ3ä†4FGL J0122.1-3004?íï»ÀT©Ù¾L×IÀ;ä¨+,ÔÀ<ì·/¡®@#%oÑ@?÷jðSº'8@m}aT®®?«ßXVÍ?þú¢ Í¿¿ÎŒm?îÀÎۚƿéX•";"+¿áW7T*#À?™Á]=¯?ÄÙRíÞ5AGNbcu1RXS J012203.6-300507?ïÃ\~ÁÝ?ŽË|§a­c?_ٜ5=—,?‹Ü©HV2?v[Y'ð«&?y+éêñ?îãÙ¿m–4?´½!Rkf?‡êsÛÐß?®]¶+Ï?—÷RØ_PÝ? Å˜ÄõâÝ?ínÌ°a"?˜&,`y^¤?s!d
ýíˆ?p&FÔ­¦?³W"<C€g?—m$…Cԇ?î'º¹áiÁ?ÅÓY—^nG?.7ȍ`z?aWsû?­f™\b?ÅÀcÚÊjÑ4FGL J0123.1+3421¿›ê€ÎçGÀ<†Â&€À:"Ž;—…ÃÀ<hÉÒ*Û@!¢Ÿ.ÙÝ,?ú~V²"<c?Àì²nì?œHÿ´øè?ßøüLl?@"dQ›©¿ìb>ƒÉM¼?ÐÛZV¢¿é̒ë)¯&¿™
?þÑ4¿ÒS^a_@'¿Ðg\…'ûAGNbll3FGL J0122.8+34231ES 0120+340?ïKÝV•r?'JÅtÇó?C8Э­=Ñ?:󒥡‹?•õýÏ¿çÞ?ßr§ºc'?ï¶<6,•£?ƒå$âÊW?(™}´s??$G4È?'ŒnãŒH?ƒkWCâ?í¯?"úaT?™íÖŽÍ?nU>»¶iÖ?Z'U¨—x…?±"YbOB?˜Ÿ%bû²N?ïLÞi?'Q³ÆÅ%?Q@W¶eÊp?E2ZË÷Tâ?ž‰Q½ÖS?'1"?ʦ£4FGL J0123.7-2311¿ßJ3æózÈÀTlÎþÖ4UÀ9ÊR:_w_À<-S±Wü@@ àÚu×È?ýmºßd?²'ØŸ¾Ì¯?˜™ظÏ{?è¹Nª@ø/Ó¯¿ð?ð¿Ü]aÚæk¿ÝI|`Mȋ¿àB¦¾EJ¿Ê¡½?6.AGNbll3FGL J0123.7-23121RXS J012338.2-231100?ïâ¬tô¾?hóvÿ¼?5†ªŒÕÚ¨?1Oé±ÓŽi?j¢¶"p…:?gl¦0?mtq±?Œ%èF
Ç¿?1àýk'ù?QÀ£fSw?€
› :9?‹0F84²þ?æÄt?Y9zÍEÆ?t'ÙŸ,™,?q3/ç ¬?¤B¶_ÙUŸ?‹—As¤•?ïIÐœ¹'?|5Öz\E¸?Z6rù
+¦?J?ÚvpǾ?•"ˆÜ×û?{&øÁo2Ï4FGL J0124.8-0625?ã62C@"æÀPõ7óŒT7À:"t•À<Œ›'8S@[ÅßȨ@'tý¾?Á¾«·ShÞ?¯Z"|ýŠ8?çi%}½ðç@ž•Ök‡
¿è[#aÙ丿䙅½nµë¿ãeØ!Ëå¿â²tý¾¿à}¯XGÀ¿ìÏñ¿öO¨AGNbll3FGL J0125.2-0627PMN J0124-0624?ïéΡG?Zº_¬{&?.êÈڎú?!ˆ"5O–?dPðc9?Yëð¿ÑØ?ïÛ3nr}ã?y'ôš²ë?K
šõ?=r²4üßV?qù'J¢÷?xþSÚ4iÄ?ïLØí?vŠv XBæ?bþmÞ*œ?N9W_;uL?"S¦Žÿ?tîÌ¿Y|?ïàá؞²%?W=#ȕÉ? ³kÐF§$?-÷
¨N?nð¤IpÆ?WW-(–4FGL J0125.3-2548¿æÄ{'ûù>ÀT'†@ €À9Û7ƒ$OÀ<wÎaøBœ@NX"¿åß@&¸0]•Ý?¶Økš,?µfmrIHž?ýS
3_¨Ý@	Ò<m™‹'?ïšáBO°Â¿áŠ6ðW'¿à¢ªßè'¿âìeïH"¿é.xMïw¿ïþ¾P¤]AGNbll3FGL J0125.4-2548PKS 0122-260?ïµzK7?v P£Ì¸?P£
¿Vça?FóU8Yb?€£ÀG_o?u0
ƒp»;?ïAƋC?¢!€TM?`– ­…?|ä âÉÍÒ?•´nö? Ä5I™5?ï(Á+Ùx?'ÜÃ";?s'«°"?sаC«•Ë?–Wªä·?zé{±áG?ïBL/mŸ?|ò"í?s¿þG‰m?d¿FÚÉ?'Æ´Ú€i³?wÏ¥ð'²è4FGL J0125.4+3200?éB{‹DIåÀ>O…r›(À:o€Ãþ¬À<\\3Ý}@륹¸rù@­"BJ'k?ö9¿‹P?ˆ?ºPVڂB@ÒL(!²,?ï½ö=	¿êÊáÛQÊοìNß+t"¿Ú%|ª¤¿é<¢¨6¿ïøHEéïAGNbcuMG3 J012541+3152?ïÛê4ÀsD?s]>ü?[wß
°¥?_£·q£Ð'?fZJÐãË?löXÝý‡š?³*?»›Ü¤ûˆ?E4dL½ÂÃ?c¥üœ˜$R?†äَiŸP?ŠTOGïÃá?îS"Î?"½¹
]â?p*C?h)Ä^fé?¨ÈÜ㽟^?'Î!ñ¤h?ï⤄«I'?[')âdÄï?RG¾Cwa?L¨Gt¬L¢?d7œ2úõÝ?U'$T4FGL J0125.7-0015¿ïÿú‹™H2ÀNó¼ÓZ…ˆÀ:>¨*VàÀ<eŒÿWc"@ôÀÙú\Ó@T‹<߄_?ÀÆÀCQŽh?µOm¦v¡È?îʾ­	c?ü©NM?ùÀ¿ÎÈ^éooÏ¿êY9W:¿éµO!ü)1¿ìn•	 º¿ïþôœõn­¿ïÊO[–AGNfsrqPKS 0122-005?ïͨ˜óêý?w™ý]Ay?X¢K=ðkñ?[÷ä¯ö†?s ¶Žf¶?tHy¬•í?íTú8†-‰?¹×W÷wß?"v§ã¥Ä?¥›@s6µ?°:"uÕªP?²rÓ¸:?ìdÃë-\¼?žÄ+Ó‹…?•«´¸)??…yC…4'ñ?·o9gÇ?š!³›ñù?í0×râˆ?¡±ö¤(ü¶?¤&…/™³™?—>Ó?ªVmY8#Î?•%Zp'4FGL J0126.0-2221?É&_<rïXÀT3 ù	kºÀ9ú¤û¨'À<^–ªÑÐB@
'èý/@Qè´k­?¸çý)áÐÀ?¼Íé'e"@Tá@ùòìòB?ïdcâ}Ž ¿åÄ ]Øù+¿æ58%á;¿ìŸõÔ-¿á:ҙ•gÜ¿ïý› Ø<ÂAGNfsrq3FGL J0126.1-2227PKS 0123-226?ïñL—(p+?\£Ï+äÀv?%VW•Jå?þ˵­y?Z´æä-U?[ÒCDÛÜ?ïÊÔï¸9e?'5ùm‰…?*³³«ìà?DÚ픹(#?y¿ê†‡=¥?Žx?á®Ï?ï%ï"ûru?'«(·Ð!Q?k&àèŒ	?ea†Óä¦Ù?—Ý3^4Ÿ­?€ðí_`?ï径ç	€?V|†©'"?3mx™ûÌO?'	\Øîs?gÓÌ·?U颤Žºh4FGL J0126.5-1553¿ì³Æ̶//ÀSæ¯ÌâÀ;-Ù8ëÙØÀ<™Zž²O@9`<*Ô?ÿþøþƒÿ?ß±‰ÚÀ?ã=:ZMS?þ'PÀô*?þÝAאË¿ï•'¾´V?ã"; g~"¿å"]9–û¿é(ª^û'¿ïý}Ú rf¿ÑÓTÛúg:AGNbcuWISEA J012708.49-155554.1?íÓî̀ø?«¡ôÛÈa?v¤Quî}?tŽ°L¬?¯ìmÁÁ6?«ɚu?íÌr‰Þ¾?³ywaõVi?Žj˜3šòŒ?ž±aˆ\h?«ž1U7‡j?¬ø0(Je?éÏ1ºÖí?¦SÁAd?¯CuZßà?•'ÁÎW5Œ?ÀòÉâ\¬J?¡×œyÅEÁ?ëýð6ˆxÊ?¥ ›æz"?‡æPŽù?…i%ÂiØ?½´JÊw+?¤—"9Pµ³4FGL J0127.1+3310?ì~§!ŽèÀ=~À¨À;MPïܹÀ<±­ÂEŠN@ wzÜÀ	ñ?ÿ:ŠÅÁ?Ñ?Ë)¬ ÚÁ?šúv~6'·?Ó°È_TÏ:?þù$f'¯j¿î̞ßS¸?ï—L¸?w¿ãþÊuÚx¿äWewS´¿Á¢@Ýîz¿âÛea-Â[AGNbllNVSS J012656+330727?ï¹R(»Òã?w'ìqJA?@[ؔý³¢?=UtW‡ú÷?€¥¸G»kÿ?vâjÅNŸ.?ï|>]™8á?Žãß"r?8…cñú"?HÛã=B
?27Ió?Ž0¿T‹?îԛ}Lá?Žõºœ¿c†?tTs0ö?eÌR·-$3?«ßËǼËÊ?(Àôâç?ïÙÇÈ/?"(à$Y8?YÀ=GúOf?R@%Õ€?¨Ú'‡U;?"H"bG4FGL J0127.2-0819¿×¸œ­äîñÀQXh‡¨ÖMÀ9…(šRýÀ<>EJŒì@°áõ(
¶@ÒD}ÞR0?²¦¶¸ŽQg?¹	ÜÞÎé@ìÜ¢,æ@¦+
DÒm?ïÿá—_,¶¿à2f9Œê¿â?™s,Û¿ã­_I;³¿äÀÉë£R¿ïüäÝdʅAGNbll3FGL J0127.1-0818PMN J0127-0821?î¥féT•'?]0­?o ×Š{Ê?i™®)ÔÊ?£¯ƒòê<?›±¢é`8-?ìu™"#$×?À`""ðÜ?¢œæôW^?³ôæ}&s?³,kl­˜?µ?æîÆX?ëó?Ð
3?¥wËì? 5"]î?)z@Š…¡?¿	Ë?Qî?¡"ü¼e¨>?ëÒªFÉA?¡µdS³¸?©Ù\%˜ó?"YÄÉý°Z?ºŽ}ÿ¶é€?™gˆÃ°*H4FGL J0127.2+0324¿ÔŽ=5ü¢dÀM ÖÓõ¶À9ëRV)ŽÀ<A¬½ã%@ª—mÅU?þƒ=¢!þX?¸–_×Öì?©"U´?òŸ£ž\w@XS­&>X¿å¶À'¢Ü¿ÁfA''–¿á,Xï
¿Ø͙ÞA¿Þ"â¨V¿âôN>aAGNbll3FGL J0127.2+0325NVSS J012713+032259?ïö`®¸?J?]ß¾ðN?oÛ·½ø?ü¿äÜÉ?Q¿s¤Ój?Hø›Û­ûµ?ïà¹"y(?yb'°°8v?$&9 m5?GÂfBÚ,ò?nˆÚ´Ð	?w˜…ªŒš?ï?í6€œÌ?z–"æ[y?bî  °8?LÀð<";?•¤…éK?xÿYCý ?ïÜR;K¹³?UPèV;'C?E1ž‰)"?œÏ~íÏ?qY͓©Ë?Uxúµ ±4FGL J0127.4-4813¿à:ò†^˜+ÀPñ(Œç°À:¡îàªÀ<±HÒé4@6\>šD@¬u>p~?½¬Žé½Hu¿›íµ^\µ?ÝxÞ8/v@[–ˆB.?Š&Ã‰à¿ééŸ"w¿å¶?A´U¿á¤•á~4¹¿ïÿü¥¬¨?ïÿÍ
	n>AGNbcuPMN J0127-4813?ï'©'±?CØÁl?X"¨Þ?Q8‰<ßp?x®Ì‡G"é?€@º°?ïœà¿ü«P?‹ó©ú¾?DqÐ7ð]?XÞOï'p?‡†ãѬ½?ŠhK:®R?îøWi,wM?"Ic$®Mî?q™wq¾·¼?n#ä£ZTž?œŽ´þhŽ?'aÅw×Ú?ïÄ58ÕP1?ha»Ð«2î?PR(eÃ#?E§Ú9×ÛB?yÐß>vý?f™àùoJÅ4FGL J0127.9+4857¿î×µþ¡}‹À*÷´ÜëÿÀ:9ƒ^ıuÀ<%'¡}"@ãþàEP@؝jßqë?½"¿Àéz¿*ò¿Gœ?Û÷ƒÈL
@v¢ÔUØ$¿Å/"Â͚}¿å"wvY"±¿ãNU}àÖo¿ê\ \–ÙÌ¿ëEMýcîg?ÖºqëÕ¦AGNbll3FGL J0127.6+4851GB6 J0128+4901?ïQ¼Ç´FG?'Zš$û?_ã68½Í?`''Û–?"Ê3¥ëZy?øTfm¡&?ïwfÇÕ?•Ÿ`ø¢‡?Fv¨'C
þ?[°œ)î)Ö?Z¨Î"í?•6W«8aä?î·Á¦±€©?8ØB³"R?zK¾l–NÚ?uËgHñ—¨?¡:mÇU+ž?‰
xÉf¡Ü?ï+ƒ?Îî9?æ㠛YÛ?b%á³.Œ?Që	ñ##?˜JÛϼxµ?~jbXò4FGL J0128.2+4400¿Ý/®|]QGÀ2^ê šª;À:ñJ¤iuÀ<gÕÈc@}"‹›)@2mæÎ?ÒÓJàxü?Þv­*@pZ:Þù@'N¤RÛ?ïùHUÚ'(¿â£«€ÌÄ¿é	¬AU¿å
" ®¡>¿ïÿ÷fÔJp?ï¢O¥YÁAGNbcuMG4 J012818+4405?îàYœ?˜ÕÊlÄ|?€ OõOÚ?zê¯'Ãþ?›ä§âäg?–5›'†9˜?ì7®ö¯D?¸tªg©Þ?£Ó•'ÚD?«ŸÁŠª?´X¿]cÛ?±§C¨n?걊fZfÖ?¥V"6Ÿð8?©á·Bÿ°?"X)™rK?½'Ñ+¬ñ>? |Ü;kj?èçývrµ?©ÙaB}ÎÄ?¨"2Ü@?"6àH¾ Ã?Æ_)²4u?§E½g¼N4FGL J0128.3+5710¿äºôœŽZeÀ^ÒàD²À:…	ËZÝÀ;ö÷ÛnP@@Ê?SÒæ@f–DzƒT?ÀË0šÁ¸¿¨tæ†Ý)f?æÊÐê°
@6hk#d‰?ä?}ïD¿á©ýýÇA¿éÖ.u^Q¿çÀÔÁÔi¿ÄÚWåD<ñ¿äMHˆ/AGNbcu2MASS J01282987+5712494?ëøƒqeÜ?µÐ~g?z¸©ƒUt¸?læO&'?¾YßGyÒ?´¼ÍL*sB?áϯƢ^?Åt'|֜â?abN"‡Ï^?uGb"ºu'?Ü=ÛՒï¦?ÅFþ0¿?êТ+ðg&?§ÀgȘ'?‰òåæƒ?yu—Zºô?ÃUñíþ?¦)Ó9?í'')0?—VمOUv?_ÍZ­$òN?Sòu
C-?¶H9¬"Â?—/'Èc4FGL J0128.5+4440¿à&nSÅ¥À1±Û˜AªÅÀ;"|úÀ<ŸÍHÏD@'³Jß@£a™x?τ"ú£tº?ÒÁqºWC@÷~0‡‡@
^~\&q"¿ïÿ	ËZÜÅ?ïþ¹ä'¼0¿à~ø=¾Òc¿àéÔå i¿âËNÀŸm¿ïýjŽê/AGNfsrq3FGL J0128.5+4430GB6 J0128+4439?ïíb•W‰_?WNÚæ®y"?E- [±ë#?@Ý~îÞª?Z¤E#I¨?R´ïò¦m?ÝWŸ"?Šš	9n?IÂO)+"×?\úۜå?Š6£·…aÓ?‰¾«³]?î8$Rb¬?'¯}5ìÏ|?ˆ
'ô¯Ì0?}´À^ã1¾?¦zpáÍâ ?‹Í#‹›9¼?îåºßR?ƒ q~r?qu
Ë!?]>]W?Ÿ [±P2?'4ʶñ4FGL J0129.0+6312?³wO8?äÇ|Ìy1À9VÚÎO¨À;(Âñ·ü@)Ûp©‹@‰‰>ÃO?ŸIO@?ÑÏᗊ @"ßBñX?þ[^¸ù?ê|Iâ¢!(¿ÜJÐÞªDã¿è+b€=¿èr(;ˆl¿ïþSÝͦ?B§D}AGNbcu3FGL J0128.4+62572MASS J01283059+6306298?ÁÚÝ,€>Ö?²Ð"်?ȾŒý"?Àí3ÛùV?åY¥užê?Ã(Bxþ}~?ÁBEqq?Û¾—ãB?¿@Sf''‡?»˜­‰#Àa?ç³åÞ±k?ÇÄùsç!}?ËõKÖoHh?ª°gýð7é?Å6gRRI?¢OžKYÎ?ãµE™S?¯ëé\‹{O?¿s\j#¹?¡€­÷*'?Ðïøޞx6?±ß™IT`?㙘lLÂ?³»môû>æ4FGL J0129.7+3436?ïÈ}?çÀ;—{Zê1bÀ:ΪcyÀ<¢|(oŠÒ@©…©	¤?üYo!öÊÍ?Ì2T¦uu"?ÑèßZ©š@ÂE¿ý±q?ü;ÓÐÍŽ¿í^¨âŒÒŒ?ïÿŠ#ÚМ¿à?(¿'ÐͿێÅ?º«¿ã;½pcj¿ïþ2Ö!ªAGNbcuTXS 0126+343?ïÖP,$?j:˜^}£?R¡kæ˵?O«‰—]G8?pK|Æ·(ü?f?¶
Î++?íƒ%õed?®\"¹B1n?ïÀ*hk?–ÑLÿðÿo?°(ìœÒŸå?§pxy?í;©f\®+?™á¨HƒÒ¢?•.x€"'Û?ˆ'+W%M?°×¬ùmð?"ˆk-7ÐÜ?ë¼î¬}mü?›É Úœ?£H[!VÃA?ªOÞ*'S?¸t]i.z?—ØÚ৽4FGL J0129.8+1440?…•ªÊå4ÀG"ÇŽŸj"À9ü¹w…r›À<UÍ&Žà@‹]†6@ø6Ã
¬+?¼÷¾=?Ňz]>J@8âe+Ô@uÏm À?áÛނ׶5¿äÄÏ"¢À¿ëSÕ£Ï(¿æü":µ´¿ïÿØ'sâP?ïýgr0õAGNfsrq3FGL J0130.8+14414C +14.06?ï[,®.Hš?˜wy²‰ [?'üøÂ?'] Ó´]°?†7Üd«Í¯?'G&€Ìg%?íËH=o0?®|ûÈð?ˆâ5:»³?"žÃ–ŠÇ?­îڌ.?§¬
l?íÑÇЍŠ?™…ósxþ?Ž.¥å}E?"ÎÚûcx™?«WÙ}Ç°'?"çdc÷{P?îÿâ—s¤Ô?ˆ¥6€ðÙ_?ˆ!e$<³f?|0ñúÛ\?"òúmÛ?€­wZwD4FGL J0130.4-2129?ì7á.:{ÀSޞ²gÇÀ;8Ov_ÙÀ<Äå°Éa@ 90ƒUŠv?þK¡ô±î$?Ê,ëš?®.‹qYM?à…{ÕctD@xUy"%i¿ïø•½ìà?ïÿèþ†®/¿æ/:€.¿Ó+u¤œ×è¿àqÏP4˺¿â•=×AGNbcu2MASS J01302573-2128389?ïï­QtrÑ?VOåuÛîŠ?'°4ª¨Ø? ¯hËÿáæ?]¯VÙ…2?U¨5"êm?ï¼2?ýu›?ƒC–(?,µˆQk'¦?A¦-®[_7?€€™ß\êï?'ר»œ¥?î…z¬îƒ?†àpâÒÀ>?l_ÅIÑq‡?WÊè>P?¥âXÜz°2?…ÔYœ©Íð?ïxÀ›«ô¨?vrßMká?SYÌÝ¡ 4?H'º\Ž?dŸyN¢1?uÖöµst4FGL J0130.6+1844¿êJõ¶ó>ÀE"C•%À:·t×Bq•À<zd׍@D§ú°`@؞wNëö?½£‰¤^¦Š<¿f?çm°r#3?ûÒÖ+›9W?ëÙßYí1¿ã¼§ñK1W¿èy6ýîü¿Ùö?¿æËxÚq3¿äã߸âµAGNbcuMG1 J013030+1843?&q+]?›î¨Ç;O°?j¤6Á+³?]7±?¤ú7±7o?›>#à($?î"+:Øïw? !¤hÑ?eŠ¿µ³àD?nÂÕ©róW?¥t Wʆ?žãØ_u?íߊ_˜zÛ?'¶ƒ=®Ì(?}÷!8'U?kB%G}µ?®Huâ±@=?I.8™t?좒^~tò?–žØ'@ ë?'H×d#A7?zö€Œ›Mí?¶™73ˆ?•]
ñM	4FGL J0131.1+6120¿ÛƒŽÇ"»¿ò¯bXº¬9À8Ê&LšãFÀ;™Ô	×ð@ œxfn?ú'ƁY0ô?«_§/"R
?´dsá½äk@mgŸKŠB@5êhi ¿ïìk˜ÕN|?ï5O؅g³¿ÒÑ@"ªt2¿Õ¼`Ï"½¿Ú\"»;*¿×fq#-×AGNbll3FGL J0131.2+6120RX J0131.0+6120?ï_uW" ?'x1~ó?Bø'èð.<?FË.DÕZ?"ˆ
=Åú¬?'ùîBì?ç°ß\q‡[?ж•!?`ú¸E|ón?…@¹±Y'?Ð|K֑÷d?Ïç¯Ä,?ì!=h¿™?£LD"e˜¢?…ØŽ*‰Q?{ÀŹ
Ÿ?¼;ô³ç?¡è.Šå"÷?îόV2Žé?…%Ê£´"L?eGHCÅ?T'¬—''??¡µ¶,'?"ŸCXùM4FGL J0131.2+5547¿îúÓÎÒ>.À›œÆtÄÀ9Ѳ–À¡EÀ<Úìô‹@	²:zOQ@Ç>'Ä?¶)G!&Á5?' Cò7?ÚÉmÝ(9°?ðìÌKós€?ëÓåjR"¿ÒD¬{*C¿ä"éœl_¿á¢>ƒÉM¼¿áèi«•D ¿á?áíEhAGNbcu3FGL J0131.3+5548TXS 0128+554?ç­÷BÙ¢ì?¼ÄS`â"?"(>µØKl?w€ì|Ë?Ðτ÷Í?¼§Z¥Cv?ÑBõ¼ï¶î?ÄÛēÁ\?žßá̺?›Ž™´ªã«?æَ"Ž#?ÄöL
Èú?è*õV#ô(?¦°nkìüÒ?›a󻜀?ƒÀ¢éL?ËçìCx»Ë?¤óÐÖ?8Ò?ᤰçç8
?°á"±K¢-?À ýÖW™?£&òÏÁc?ÔfE›?­´@ŒO4FGL J0132.7-1654?™`ñPÀS0#̎À8qŽ©{ŽíÀ;âêJŒM@»ãr€¦@&ÝA‰?œS蛛¡?¯" î@UL}‡\@:T‡–·½?¨­[ î*H¿âgwÞ]îÉ¿å"Â<Pg¿åfÿš6¿æ-À×K+¿ïÿƒ}ùUAGNfsrq3FGL J0132.6-1655PKS 0130-17?ïÍnì´\Æ?oõ¨0}r9?MÁ^MvÐ?Cà'ÿC)?u¦1zî'?n+ß;«?ï¼Ö)lT?‰šóEÚtö?9ÞçG.9?djÇ ??öýVñ…?†{¡RÝ?P?ï ßkž‡?…'0=t¦?s©‡ÅÅì;?mg×ÑM?–ù°š½¤‡?ƒqbq$?ïñ öS¾?I|1¿ç
²?,".øŸT?%]_X.Á?Y+yoï¿?G5³$þx4FGL J0132.7-0804?ÖÆànÄÀQ%EŒÒ
úÀ:½%eëdÀ<{Y"M@ >_W(…Û?ü4sT‹r?ÆlN'^?ÂÌP{£`?ý9ƒ)Ì@?ûdÚ­‹¿ïÿù&Çë?ïüe@Ìxê¿«{ŒDg}¿ß,ÐÃ|l¿âªo¥Ó¿ßæ‹d͊AGNbcu3FGL J0132.5-0802PKS 0130-083?ï~6´qœ@?ƒÀ¼4$k?NN"œ"i?E²q å"Ü?Žj™×7¼?ƒ5»öl½ ?ï5[î'ӏ?™«JLÍm?bWwYØx?pPuí§v_?—	"B"rú?—.óÇ_·?îc6€eâ?ÀCEC•V?ucI""?bN)OŒ?«]l.ÇÙ?‹Ì)ü¦?쳛€±"À?™LâLåà?…Õº/<R?v4qALF?·¨l´ŒOª?˜FæGîÉ4FGL J0132.8-4413¿ïòÇhúÀQ¿!>>)0À:W]$žDúÀ<¬wD@œÒá¹ÃÜ@"¡ã6ï?³"jŽSš¿«¾Ùo˜g?÷ûƒ™}?üSÙÆÛF¿ÕéC¥ò¿ç5ø¿ßHƒ|vÉ
¿ãÒ. ý;*¿è›_Óû?Ðؗ;ˆBAGNbll3FGL J0133.0-4413SUMSS J013306-441422?ëCüÿJ?À-Açc
©?ƒ9+S è?~ƒ
3˜O?Á¼{BÑèÙ?¿åàRŒ†Z?îْ0 ôU? 
(/ø••?s|É9l?ƒNÑ¥*Þ?Ÿî‡œ?›R‹Ù>Ã?ì䁙"B?™û´oÒÆ?Ý¬iaü?ƒ§¤ç"?´¤ˆ-€½m?•'còÕM?î9—ÜkUß?'úö¶<30?ˆ9âzn)?{Dca¦µa?¦X	šÅƌ?µD$dä74FGL J0132.8+4324?Þnr4¶ýÀ2ÔUGZ2À:œ½‡µk‡À<~ÝW^‹§@Ÿ™¯i·@|¦ˆÃ?Å覺YX?ÏèªäD¸—@*%£'·Õ@Q»úA¥¿êN›n…ð?×ò)é•ö¿æÜ¢˜E܃¿è6'@Œ¿ç¯§"X¼¿Ò6ÓfD¸AGNbcu3FGL J0133.3+4324B3 0129+431?ìP âÅ[?´(Y4"ŽÍ?Œ•%._Ê?‡´FD8k?¹ìZ›Ûë?²çƒ5ÆÓ?îÊD὿F?Ÿv6'­à?s\PË?zŒÊÔ?L´? êX£ÁŠ?œn@0«²?ìƒc
Fšv?øb¡d?›aÔw äË?‹–ì<œ<K?µrwâó ?•ˆ(ÛWø?îyH©M?‰ƒ¥€.¢?'Vˆrð¼˜?wÊV ‹O?¥=';òд?‡V՗¦òG4FGL J0133.1-5201?æôþ>VIZÀOó'½RÀ8¸_b"À<Ûä—Ä­@a–8¼@ÐlÚ"?¡¹nÝ>›,?´ØœŽÁy]@}<y-ˆ@zdËÍ¿¸tsß²¿á%ĵ§Z¿åŒÙ݁zê¿äIê.Ýc¿ç-""aSØ¿ïÿGþò8íAGNfsrq3FGL J0133.2-5159PKS 0131-522?ïÚ¢¯N'_?iã‰}Ñ&?OC"sZñ?Fî$1+|;?mŒˆ·	O?h/¾àP¶º?ïß0Ëûbâ?xppo??#_j_êd´??ÃtçoÁ?o™=^žw‰?wú
hæ4g?ïDJÙXbê?…¾½""S?qLí.å?p#¿b:¶'?"#Ÿ§él?ƒ¡M£h?ïþ"®4˜? æ?Œl>ðuP#/>ï%ªÆ*f™?,8,tñ? 	ô¼¯U4FGL J0133.2-4533?˖Bï`BÀQrŸ˜·À;·.Hè§À<ÿ'zç&ë@!Í\áb0?ìišÎM?å‹ÿ'=?åÓ°ìœuí?þëªX-¾?ò'.䬿ÙäŨ¹?í,{ž†é>¿í¤.}ÁÌ¿?ÒÄîý#VÇ¿Ö+ò¢xf¿Õ>ºÛˆ§YAGNbcu1RXS J013308.8-453528?ín#°C'?³‹ãEgd?"1O½}à?†—±¡få/?²¸›¿É?²1Ɖü?îÚ³ZÌV?¨¶ÖD?x&Ógš ?'ÈûÌ}Ü?ž¨Êñ›Y?¢–°5gÚ{?ì;ú5'Bö?Ÿj¤±_œG?"ß¡x&®?ˆ'/À¹‰E?¸èEõäDl?œ¤_±¸LX?뿦
Ct¾?¯6#½Êþ?n(&çg_"?|֐‰òç?ÀˆÇ;TŒ?®öï;åº4FGL J0134.3-3842¿å˜PDw9"ÀR֜wškQÀ:í—û3èeÀ<ÆÝåùÄ}@åçØkç@n£f¡õ‰?ÅEp!¦?ºd]þ7ÿ?ñ oÇ88V@-âÃJb¿ÎY	†'¿ÖZ–d
0¿çD[C¢¿å[«!Z¿ïý¶¿oA+¿ïþë-
$FAGNfsrq3FGL J0134.3-3842PMN J0134-3843?ïñÍ4V(?`hî3Î?7Eeÿ–†?6
y›ww‰?V">Yn
À?]id߅ý?ï±8±§M?‡ Ólù³Y?>ÞÁHmÎ"?W"YŽno?'ºé‰R¾~?…Mf|HÀ?îú¸[`EÜ?…U¶K
G£?u×ÞÆÊa?pŽ¨ÊÇG?›3.\E'?'Œï¦*Ýh?ïÁ–]3õj?eh"–€2l?R9!0ùÁ?BË
­K«/?z¦‰Ý¹­?dWîïä"4FGL J0134.5+2637¿î8B]¨ÀA oÞµ,À9U"¢ß"yÀ<
:䜸@@‰°îIõ?ÿ@7þtÆ?±:Çw"?šTg¥™H?ésñ~Ý֊@EZ¨6¿¸³ÿÌS€¿æÀ|ôGe¿ãÚpßf,…¿Ï‹Íþûô¿ã7a@6ÑοâV¢8¤Œ<AGNfsrq3FGL J0134.5+2638RX J0134.4+2638?îxãFv?ùe´?h6î­|Í?^=¾ý©Ê×?¦~ž` À¸?œ! Ê¥'ß?îÔàUÅIè?£Sê~€ÿ?`»J&ôf?u¦åp_?¡¦I_ò*?¢‹I]'þ ?ë¦þÉ$Ä6?¢"rshA?!,ìV?}Ûö´×œ?¿#ä3¼Sƒ? ÃND¡Þ‰?íX64·E*?—˜†ôã?†ßˀÆà±?sø¤Qóي?²bTê,úš?•wy³
4FGL J0135.0+5338¿é¢V"ê»ÔÀ!^3‹GÇ?À;&ԅ'òÀ<´¯L¤@#hŸ§@Kj¿'zç?ԙ¨}b+n?æý6Œ"a@×'j@@ñ#
Ì?ïýÚ¡K¿œ¿Åz‡Á…Ç¿áû3¢™Èi¿ëß3םá'¿ïÿú÷''ý?ä™'¥RAGNbcuLQAC 023+053?ÙLñ€`}t?ÅÓYÕt?·!,ƒ²8!?¶—?˜ù—?àua¯YzC?ƶ½âÈ?Îàî<™èu?ÇqÿËKé?Àü–F?¨N¶ÒŒ?ä¼Ðsô??Êùw¡¶}è?ݿ̹C*#?²9Ĕ•j"?ÏIA8¡s]?°éï´ÃÙ?қ'ªl/?ª`>;€?߇‰0ô=y?³Ë8L"?Î"C²v'?´@û;çc?Ñp--2‡??±ú½¢Ú£4FGL J0135.1+0255?êó•I¹îŠÀM½º
RiÀ;w³Š§àÀ<­ÓÀÜÕ@"[ÌÚ
Òü?ùYÝÿôB?ÍoÃ\`©
?´~!sBB?éSme^(ª@(â@Q~οïþš9҉¥¿¹³BVä?ïüùðòF¿Öצ$lpì¿ïé
?ƒ£Ž?ïгâ;ëAGNbcu1RXS J013506.7+025558?ïñâÏÂôÆ?WL×~m-?"zë9ý±¤?#ÑH"¿ôT?YëÖ¼v?VL­µ5Ô?ïœ=ÿÖÝ?Ý·Ã?@FÛª‹Ñ?ZrŠG´Ç?‡ø'ΟŸõ?‹t]±Ž§Æ?í¬:žJ§A?˜–×±0?‡"èÈhT?ƒ¹›<?¯{±!#qî?–ŒÆxgœm?îìj¼ç?‹3±sž?Hså|ì?Lá­þäãÉ? ÖĪ?£?ŠõÒÃÍ/4FGL J0136.5+3906?ìuŠzåïÀ6ðMDVq&À7´åÏxyÀ;<Ðjæÿ@"n×S9?øû"}ö¦?š›œÂݤz?´û0f…p@Õèc+Hƒ@uU6=SÈ?ïû!>>)0¿Ë»Cs¿×Ëw!ʀ¿ÑW8 ,ñ%¿Ö˜Ç¢"¿âCÖNUÎiAGNbll3FGL J0136.5+3905B3 0133+388?ï"Ñ'¥m?ˆ>.ÏÇ$?_£‹y¬…¨?d
1§£nÜ?‡*'o+?…ÜŠ™ïç?îáà ÁÙ?¢IÓûGè?x"‹m|?‹ßæ q?×f"Déf?ž§-Û?ëMôÆ6T?¬î–
Z#?¢Â‰"ô–?šùžH³A?¼/P‰»á½?©7‡üœûÂ?ë
»©Ó|?®pÞÌÕì?†ºÝDÜ?z6VΧ?Â]oÚßlO?®"Oßd<'4FGL J0137.0+4751?Ú:ÔBYcÀ,žß?–À8	wíwg@À;–ϲZZ¿@"58$t@'ßƤ"Ÿ?œºâ"Š;-?¹E6€o§@Ÿ
âµ@¹õ"¦î¿É8ÄA¸Ý¿àiˆ†a¿äªg|æÛl¿ã÷±j8X¿é!ÔfB¿ë|辚ÚâAGNfsrq3FGL J0137.0+4752OC 457?ùè³Þ?gûÛäç?[)ÃÂû?Zm…Ûã³­?‹ö<MZÅ?|U¢\
¨T?ï²½;vh?r–ùAø$?O+n÷1‡?e›5æÙM^?]ú3Mx?ŽQqéK?ïiÁ9 ÁÔ?}Íí ''†?u¬ò±3'Å?rMçÚ®ÚK?Š¹8?5ə?uEß(?ïëŸúÙÝÏ?T²¸ëŒÁ?5@(Ja>g?+ˆˆ{,¶ë?a¸Ö	#?Sef'ýà4FGL J0137.6-2430?î;)öTVÀSÒaAcwŸÀ9ɇî"À<BÎxžw@¿aj~#@@E®_ú?¨£,ëEˆË?½¨Ù'¤Þ@«c|§Œ@[òPêԿž¡{eQ¿ã2†óпçWã줩¿éž¥2¿êÌÝÿ$7î¿ïÿŠYŠµÑAGNfsrq3FGL J0137.6-2430PKS 0135-247?îà›
£?ÂÐ_EdrY?LV0´ê?Hg¤'CóÌ?¡"ïçc
?ÂÔvz'œ?ïÅ-žÃÿt?ƒYöz'n?4/,I#ÿ¥?M"›ÖKݶ?|&=Ùnï?'Œrë¯yß?îúE'sbØ?)*… Ûv?'\SÚ?€%GòŒÚ?—¨!¦ê†?ˆÂÑp¯?ïú'¶·™?48KÁ¹N?"VGbw×?.Y[Ë)§?A$/Lƒ¡?1ßùy:¼4FGL J0137.9+5814¿ïA/¹ðÁÀFïÃqÚ8À8Î3œ¾àÀ;ÊÖyù@ -ÐH'OÑ?þø–IƒÑ?¦ZßZÕ?Žà8±Ä«
?çé‡=G@úºÈ}Ü¿èQu¾sпԳµ'k€¿àħš
\à¿Ý
ˆïþ*=¿àÅ+<¿ØO*ÀH&AGNbll3FGL J0137.8+5813TXS 0134+579?ï€-‰ôü¶?":ßÖÀ¿û?8'cŸ¢Úù?2Þì¬ëO?0
eû‡?ƒáBEÙ>Á?ë"Ò9Ä	Â?¾>i®É û?Eûç;?\HþÒ1lŽ?Á×'óñÞ?¾+wq|·?íyÂæíƒ?—ɸrπ?z'ñd«o
?oTôÆSÜR?²‰À}Üú?–§'½¬ç?îß-ÍÚÿO?‰ü+‰$/?k¿{y­Í?[:¾	¤ry? Q+jµ.>?ˆMCÁÄ-«4FGL J0138.0+2247?·Åbª'³ÀCi:2?îÀ:%:G#«À<R÷eýŠÛ@²xà;"@}æOU?¸6Îs@–?q8áh¨E?ºS²ÚˆL?@z÷NU£?ì³åªê#ö¿ç^æªÄdH¿â ÿõEq¿ÖÄÀŽÐ軿äy-Œ*E¿ËgIû¡¡{AGNbllGB6 J0138+2248?ïÝjƹÝY?g"Š}%~?5]¢TÙVj?.ê¡p•ÃH?oé"û‡|V?e¬û¡úVÀ?ïƺÞካ?€1F9­?"©Áoøq—?:ð<¼^?|
Bƒºæ³?·Ñ1U?ï&iåÍêL?|Ä:
üM?`ýéÙÕ?IVg'™?™ Â?{…÷t¤Ö‰?ï›òòÜ9?jðP¿«å>?GOqH?4=£q¾~?‡ŽñÁßô?j[Ùr6®4FGL J0138.5-4613¿í¸";¥ŒÀQ0DR?gõÀ:j&Ñ%!"À<¤×%+3@îrì û@î¨|‹kÙ?¹õìUÔ?œ'Ý<Ü?ãªJè\?øs™)Ý?ïï
3Å)j¿¹ß#¦@¿çǃ·°¿Ù@X *,y¿à9¢cÑ¿ê	Ý>_SAGNbcu3FGL J0138.5-4612PMN J0138-4614?ïNB%ìÐ?‰RT7³?Z¿g\D?Sœ53,î?"‹ÊiL¤r?ˆÈ0¹O2?îûé¶Éóæ? Ôð,Ýx?f¸Vvk"?sÄݨfˉ?«¾d'µè?žôÌ3ö?íŠoLŒ x?'~'%ý?ƒ;;ê¾uÅ?r®+%%-Ò?±EC-?iºŽItá?í)ÕE k?˜æÙM"Ü?˜Z"n\›?ˆòwûzø?°šÎr!€?"»¸á½]4FGL J0139.0+2601¿àώP:UÀAϋ«`kÀ:´•ë/³À<8;-Ówâ@@,ôÄ0@"ÅDBO0?Í_á'¿'Õtß'¡?Íw,‡G‡~@¡¤ì³òá¿ë>øcSŒo¿à_*g²–Á¿Ûétƒ	µ6¿èBÜôb=¿àÒ\XÆ¿ïþ­…èÝAGNbllWISE J013859.14+260015.7?ï¼Ø¦µ?}EhO¸Ÿ?Lub'àcF?Cñ¬Zc>Œ?~¢iq?|ÄûYC¾?ï](Ûñ?ò?–¥eé‹i?CÚɾðª?]¾'¶Vé?"Áõ«Š
J?•›'Q®Z²?î'Æe'?':M+þ°?|:Jُïî?v¡Ó¼˜[?¤X†˜g¨Ü?Œò%Õ0Î;?îùِuÍÍ?Øs̸åé?L˜iÒ0¶%?A/+ÿâ€?Ÿà
¢´Àž?²°ÑÿßÒ4FGL J0140.6-0758?ë'má@2†ÀPäýó¶E¢À;¤ÍªB^À<™€'a–ô@ ÁŠ^"3N?ú¦¯ç¹¸?њ'ÇÅý?¢nªW¬å?óÝ­ûPm×@KŸ	0¿ìèiÿ#â?Ì:OMw¿×wS´Eí¿à­'f¿½›Á'¿êøC""~AGNbllRX J0140.7-0758?ï¡ÿŠì?zxv FK·?C¼&!I?<b=S×)S?†DzÕlâ»?y¡ÿgä	ž?ï·:<z=€?"þüF?33Ç÷ü"
?Jǔþ z†?—Ò¡°»E?"Cg¶\º€?î+O×`Å?EyËtæ?nþPëã?`+mU
R?«^F©"ú?ËôÅl†È?ï¢ÇXW?€×MFäÒ?5…»A`'?1l
M~Æ?›õ'ù´g?€Æ:Ks¿24FGL J0140.6+8736¿â
ëøm@8ÉÒ¿UÀ:ҏØO·ÎÀ<A(¿<@ ï>fÃ?ÿy)L)¤>?Ç)×iÞÀë?¾ä0ì†ü^?ö®×ï?¾@
ç¿P7zì?ï(šÞ"ԿۏÔ>0<^¿Úõt,öƒ¿Ü/ö$_¿æ¾­OY§¿ÑHÈÆ­ÎÛAGNbcu3FGL J0139.9+8735WN B0126.6+8722?Q½3?}5'0¦m£?FW©xó??Gyå`Ïx?‰°F°þËé?|'…dÛx?öàú?‡!|Ò­?I!§/?Ue[yk?Ž§Þ"ÏŒ?…×4šÉ»?îǖ"QŠ'?‡cß½²
4?f¸n6Ô?S\b'Ð:j?¢çz,?†Pd˜V€?î¢k%(Z?†4•-cp?qQi<õO?X1GF^?£¸C€WÛ­?†O齚Y¨4FGL J0141.4-0928¿ÙÔÆ`¢GÀQ1=Ùb·À8wŒE@ƒÀ;¯p"½'Æ@?mà-QÈ@²ƒ\@s? Nší¬–L?¨]ã#ë@ò*ڟg@0;'b|¿´#ŽûZÿ«¿Ý¡+>E[¿ãÓþð5ˆ¿âh·¿I~¿äàӟ¤Ë|¿â#*!;¹êAGNbll3FGL J0141.4-0929PKS 0139-09?ïÂ~Öv	2?tCíQèê?,ЦiÔÐ?#sÇÑ?ԏ?}Ú'®çº?t	ÎÁˆã?ïÛ¦¦}KM?y*¡"}±ÿ?%K鲁ôË?F-øVtò?q'MsÆJ?x1"Ë'Ë?ï"z:`á?"Ü(½ÁÐm?n»9G·N?f"G×¹ã|?—è	¼úG?'˜%fÄkš?ïï™Î¥ô?Nò-*¥"Ç?Ý4'ȍ?
i½¦J?_~¬‡—²?NqY‡g·4FGL J0142.7-0543¿âküc¤{ÀPWÁ~ºñÀ;c1'À8À<±ÇÞP'Ï@JB•ü¬@3çÞ¡
§?Å?Ò(z#?ªqáÄ«–?äuòËd@Yï>½?ï÷®»iοä¿<Uñ¤¿ãʶ!œÁ¿è´¾c'˜¿Ëšã†!¿ïÿ~À¥L*AGNbllPKS 0140-059?ï¹ÀÆnÒ?x^¾28?HÝÏiDÍñ?Bò`pµ_È?€.r×Ïþµ?wbμLVB?íÈ?ŠæB믆¡?<êí²¾…Ì?R‡Ü@$ƕ?†+­N%Ú?‰ªñ²&™è?î´ò¦0êh?Šø­åäh?iÒ¥csé<?X˜2ŽÊã4?£«Fºæ?‰ÒK´?ï'dãŽf?uj!ÀlV?Aa|½B·?:ߤˆˆ[?ŽfÕ¯P'O?uPT®ª4FGL J0143.1-3622?ÊîÛ%2rÀRê–=Ć­À:Ìí¨À<"±ö‡±:@?þþMMf@qßƤ"Ÿ?¶áÓÞÓ¤F?»Æñ@Ÿ'g@.eÙx¬º@Q)¶1Õ»?ï÷XÇAr'¿åÀÇ`QN|¿ç!¼¿ænBÓº&Ø¿ìqT h«:¿ïþ–=Ć­AGNbcuPMN J0143-3623?ï¶[71d?¨5.Œ‡?BCDU x?L7{Cz>¸?DýôažÏ?¨5°J…Ç=?ïÓkä"_?}Ï9'»ÐO?-:Eov?K+"ÓZà°?uaT,'U!?{Õs «n?ïK(§`–j?{•B
ù²J?n%×âÝ?e!@*-?'Ù	/26h?wF‡·|lÈ?ï돂Ž–O?PTxhH#??õ
aÛD?0ŒMk9…?`qÜ%FÖ3?M:܇p]4FGL J0143.5-3156?îg,"âqéÀSköU\RçÀ;È~‰rÛÀ<´Zåÿ£º@Eöê,¯@E]D~µ?¿"/?]¸î¿·(p«¯Ç?öî |wJ?ýàÆúOçÊ?ìÒvÅY;¿æ2eByø¿çÅÅqŽ¹¿çš×Q‹
¿ãµíB
@°¿ïø:¿¯#AGNbcuPKS 0140-322?ï³Uéî?'ynæPo?Sü
#x[?Gƀ¸TcA?€«:e5F?ü²Ÿ<rÇ?ï3?ÙÀGa?¡H·ik5?\p¼›]û?s3ZƒÏ"¼?—ÐøþAC8?žÃu\3r‹?íîºbz?"w¨á +{?úퟻ?pî»ÈnP?¬ŸÓ<kð?'×·)ÑÈ?zW>
?Ž¿k9'?y8?¬øöS?p‡žX€ã?£
Pdí¤?ŒT…\/4FGL J0143.7-5846?Á¢Ìύ,µÀL‰A|¢À9	ëîÑÀ;òˎkß@/Y®2'?üz}Å'¼Ý?¥%þþ^{?¦Ì7ógä@n:p>V@Çc,Ë2?ïüX`iLJ¿Ô["©¤¿Û÷cÏ2X¿ÜR²à£¿ßŒ.Â5D0¿Ò6ƒµ+ÆWAGNbll3FGL J0143.7-5845SUMSS J014347-584550?ïÏBP Ì?°¯Eåە?}†)Ö£Y#?®
;cZä?s'5LA?›+UÕ9Ùõ?ïÍ^~\Zý?|Ú¬-™P?-ý'Bœ?AZ"µv"?xhHéoi?{¹"ƒ^?îûñ…Û]?ƒÑŽTdÆM?kû7>XÀ2?b"Uþ¿?hwY|A?'ïÇü¹Þ?ïkл?c'?uïšhá¯K?UÃõ™°‹™?D|Ã7Úl?')©>x'}?tÿï·>i4FGL J0144.6+2705?â'ààUÚÀA%ú](ÐÀ7¢½	á*RÀ;[.ÿÇËÜ@‡âÏmý@C`Ðԙ?•s‹½ãÐÊ?µ€À)¦@ â ÊæBÀ@K)<d_P?œº×+öS¿Ûü@Ã>®'¿âIÆ×p•¿áÍE˜…¿æÒí­íäu¿ç³Ø>ð֗AGNbll3FGL J0144.6+2705TXS 0141+268?ï"
óì¡?¾N–1[þ?P¦[¦ ‹?K'ûjr#˜?ˆý9böW?.r»‹†:?ïÚ?ÒG--æS?nÍï( ­ ?"®™ Š•M?›"ÿªt?šéÌmoJ…?ï!—,!?‡ <2?‡<vÈÍMÓ?…H-ŸÖæê?"¿àh³Ôð?†ñúvšË?îú¿ –{¿?‡K,L3c_?y4£¹‰?oÂ-¬Zâ?š["B%×?ƒãÂrj/4FGL J0145.0-2732¿Öù#Õº"ÀS†KâCÀ9Xy˜rR-À<^ûE†@'‹öî´S@×EB<?¯½dác'?¸ÆÌ,¾Ïß@Ï¡·uM@ÉñS"ÒŠ¿Ø?$=È¿ä¦$Ÿòy¿ç»Þ¯¨Ð¿ê˜£?_¼S¿ífà‰Ã
¿î½Þ¨v¬AGNfsrq3FGL J0145.1-2732PKS 0142-278?ïÐ]u‡f›?aҒ£‰?:ÿVçø}?3õ4f†g?v!S–Þ4?`ÿ ó; ?ïÕ¬•A"?|œžØC£?-ÏEåiå?MS^qN1ß?t<Æäï‹I?z¿ÍS
…Z?ï+!²((?î€Q_¾?pÖ_œɘ?e^Ž­J?–fD¹È{?Ù×Í@{"?ïþºªµ8,?é!2kNû>듳p0ZØ>çìŒõX?"œuzGY?Y'±²+×4FGL J0145.9+2319?êq a}ïÀBì앿ðEÀ:ÏÓØZÀ<[‰2CI+@Ýyý@žÉý³ø?Ç·.jv–_?·jªÃ¸|?îzÜ?0—x@8'ÁÞÝ¿ã7=N?(4¿½x³š÷'ž¿ç=Fý•lŽ¿çLƂ/ð‰¿àɺ^5?}¿ïþP§ETAGNbcuTXS 0143+230?î÷u0"<ÿ?–Üvlq>?`ƒÍ"cf?mƒ‡SJ—?Ÿà;ÿE?•ãäåMãÑ?ïZµ+»Úè?'ýFý,_3?Bçìà¦@?Tؽ¤¸t?"!pú?'.žv"?íã
â¤â+?'[ž6F¥?€ðÃéZs ?mþ×KcŠ?­" Û[@Š?	€ö=P…?îõ*ðÌ`?€™•²'"?aXJúË?Pö¦L¼ë?Ÿ/'ý£Ÿ?€ké4FGL J0146.0-6746?ï¼ÈÒä‹RÀHBòù‡?ûÀ:$"çƒ1xÀ<"Ö«rßñ@#¿ÆÿÙ??ÿD¶Ê,	?¸\ǁ3qG?¾E¿&ñÜQ@·Üz¿¹¿@|š	Öîd?ÚÀïÿÕÙ¿Êèà©£}¿Ûú©ÿÿáр´¿çÊäÊðS»¿àów[0AGNbcu3FGL J0146.4-6746SUMSS J014554-674646?ïãûBæ¹ú?š\¾'‹¸Ô?AFÉ{õ•?<{…
j¹?g³
ºÈÑ?š]'†;?ﶂïå è?…øz5¾?51µU=~?Kq§c¤lË?µ¶[íݗ?"á|f´š?ï9a6r;T?}¬5]	?nZ<0^?kJ\z´8C?•íê2ƒ¡?vÁ¤ðSå?ï´BðÖV?fø¯%·¸?\éMýái?Gú'ä>Ÿ'?~¤4RT?dç'!'i;4FGL J0146.3+4606?å¢Ì¢ý½ÓÀ/j²[1~þÀ:ʄս6WÀ<"Ä'k§ï@VÖüPž?ÿå€éŸk?ÇD×àÒ\?Çaá†îQ?ý¹áˆE´??û™R.v
?ïäY!bü¿Ñ²mÛ¥­¤¿àQøPV¿âÌÅ«p[³¿ã%™'¥R¿åAmž%øAGNbcuB3 0143+458?î\Äc"¡?¥;ÒÙòð"?yò‡ï Q?uf+p*z?¦õhÈÊ«ï?¤Ÿæn\:?î<Æ«?¥YU
eê?€6ûÓöÄW?…M…éa
?«~w.—ƒ?¢ÂíÜ0î?í›T-aè¤?'–ø9ȋ?†}n¬®?yA§½ˆhß?°U°Ñ0¥R?"¬(Ì?êžd¿
±Í?–t¡ª''¬?£JNÇ®?‰Š<øGÄZ?À³Ù~á?•ƒ£žt&4FGL J0146.9-5202?Ô~¯9‹ÀO~÷üü?À:aØ›ïµÀ<!Õ<Ý×@h <K	ê?ÿUûµ¤a?À®I)ʍ?½>[/{˜¨?þ"T8fxÛ@P×8`™ž¿ëc>Ò¤?ÇA»Y¿á»Ëǔ¿ß¥áË·y¿ÞËSûÕ£á¿ïô`{?çAGNbll3FGL J0147.0-5204PKS 0144-522?ïžþœ8ƒ?{ۃߐÐ?ZÂ?‰6?Q}òI}>?"è1§Áø¼?z¶%ö§dŒ?ïa|Hp‹?"r÷†"'?V(\¶?doú"|Ú?'mñ0Ýs
?"\þ…dN?íü-ƒŽ!,?¹TÂ
ÿ?%©gOMf?tˆ'š¸c?«ó½mJ×?á¡L•?î'ÎSÜ¢?ˆeSJãþ
?€~²1—$?n#'¬‰·?¢³•U±à?…Îs²Z&Ñ4FGL J0147.7-1321?ïŽ6텈ÀQ½×¡<%JÀ;i™ù:éáÀ<ÐI4&x:@Ë{uÂ#ü@Œ¶â¼y?Ú#<E*¬|? ú¶j	ß?Ä¦ý/k?ÿÀN²º¢?ïú
'Íx¿èå).‰¿â;¡–¾¿Óšß_ ¡á¿é~lLYtæ¿ïÿúŒ"¸'AGNbcuNVSS J014804-132019?ïæ'Á²V‰?c-cß?;	T °"?9֋Ëw=7?fw¹"dû?anéMúâ?ïè/8ã:?çm2¤?H}dÿÃ?YPþc:Ês?þ#û†?Žx»"úf?î"ò»7à?Sç6jëu?|5JÞ
?r0ŸŸ‹G¨?ª³Š*úf-?Œt¬N6›°?ï?´e¶6?ƒ1–Ü6A?R	ýG¸Q?NŽ¹5ç±r?–èÜÂ$½Ž?'ø&Í}=Þ4FGL J0148.2+5201?ïY¶ØðÀ#¾åGÆÀ9³EB<À<!»¹@ ¹%ô†O:?û^SEÎ@?´lŸe‹u?¹—½÷FóÚ@Tù¯ƒç@FI»_è¿ïýè~;?ïÿõÿ 1#¿Ä")Èü3¿ÜX
Ã}m¿¿Û¼ýÌÉó¿ÕÅi@¶SAGNbll3FGL J0148.3+5200GB6 J0148+5202?ïU°÷ˆ
‹?ýª×4qL?VC!_O™?Rµ!û?"å®ý8¹?{‡á{@?îOn:üŸ?´fJ–'p‰?a0F³Ø4?s¤lŸb@É?©öå˜"?´;"0C{?ìW¬^ÿ? ?0Ö˜?‰°`4š6?yï}œØ?»ÿ6™!pN?œÃrW"B÷?í‡81¥q?'•…@"?¦b+&…?|£…û?¯¥VdZß7?~ðd÷œ4FGL J0148.6+0127?ïºrahÈ
ÀM"!ÄuæÀ:q'ùCM]À<e€<ÑA§@T˜Û-¸ @Ê¡C²x?·­®¤m³¿­Œ^Æù"?öq?|Ì@Ãú³ºØ?ïzÁҝÇ&¿èmÎÜd¿ålXï
¿àæY›|Ȩ¿Ù¢†,Ù¿ïú?̞©¤AGNbll3FGL J0148.6+0128PMN J0148+0129?ïÇY‡Vn˜?tÃ@hÞ?Q•k¢þÿ?Fõ²ÎýÃM?xùßô?r~ü¶GÑ?ï°!¿uþ?…ôycg?44gÿS՝?OMmJ?ƒ]ÔP'â?"ù|/·0ƒ?î¡r³ÿÏK?ŒnpQÖ®w?pZÐďË?a0K—â¿Ë?£Ýz§q–?‰ìÔèR‡?ïFƒ@ËÓ?{–UÝ)Ú/?aLj͎?R$Uhíõ?•
Ô?zï¤É¡_ž4FGL J0149.6-0734¿ê¥ue»NSÀP… …±…À;L;æ`ÊÀ<§Ö»cý@Eûxö@Èïþ*<ê?ÒEè8¹?ÃØEç?ê§?ñ"ì~Bûþ?úü,ý~?ï³@S'D¿Ë»5À¬-¿èåTƒ¿ãÅ©!ÌÙb¿ïþ
¡ÿÏ¿ìRÍAç«öAGNbcuPMN J0149-0733?ïsÁfÉ9? «žHß·¯?`2`AŠ_?Z'÷9X~?=[Ú? žD-Äj?îdEíúi?«ùíwÃ#?€tӇŸò?Œ&{ÀY×?¥žœúþqx?¦½°нÙ?í-ÅÍ9Ù¶?˜öKRŠšd?'Þ®÷ZñÇ?ƒÍht®B?±Ú%ØZuÒ?"vQ?ê~'åGJ?£†ƒr´ÜÏ?›–˜ÑPm?‰W&=$?"!P¹­h?¢ìýß¼•4FGL J0150.6-5448¿ï_†DʂÀN%db€'ÙÀ;K¹Z)ABÀ<ëªfpw@ #Œ¤ÄS?ùÃԅþ²"?ÓñýwŠ%?Ï*y¦41¶?ôm3	AÈ?ýî¦un¿Ò‰÷Dðtó¿êÖc"3ÖÇ¿ßü^ Ia¿Êç‰¼'¿çÕT{ç¿Àψ=üÞAGNbcu3FGL J0150.5-5447PMN J0150-5450?ïXÖ­›ª%?‡+àl¢Y?RpKÓ®ï?D×ïñ,þE?"¾%OÙù?†À_
'È—?ïGÞYr?—ˆ/u?Yuty,h?jߙüqÑÇ?•låVƒÞä?•5°0vÍ}?헦DÑP?•¥mrVñ:?ãÞ4ý4?u˜âu92æ?±S×XÕÕ?"°|©)m?íŽ
åÖÎ?—/Ü)Ãc?eZ†÷Vs?ZHaŒ":?²æüD™Žä?–µ
h¶:O4FGL J0151.0+0539¿Õ3µ¼1kÀK—þŽæ¸À:Á'ï2RÀ<mwVx²™@ӀÖ)Aî@ßûH
ZÍ?»ϘY'º¿²à#–³
Y?øq‹'æÎ×?þRP6ú*?ïú¦$¿ëÆíàBËW¿çt‡>.¿ÒbÌéR>'¿Ú§½ž±†u¿ïÿülòAGNbcu3FGL J0151.0+0537PMN J0151+0540?ï}Y*œ"‰?†¶X
¿?c7~˜·?\¨¹0j¢?‹æ§y4°j?…	ƒä5?îýDP-$?žj$öhÜ?`'ZlÓ¡?näš•Mœ?žG*¬Ý??œû.
o?í¯JäOT?';Á׶>O?~'
Nž½€?k=œà±+Ÿ?°œ˜›sC?'`)ǟFw?쳉ZˆH?mêÜ«¥¥?"n‡VF?vÙHrö©
?·âGZÒöŒ?›ø¦Ëw"Î4FGL J0151.3+8601¿¥gÏ6Ó^‰@7GM3H,À:´4çhÀ<h23Xòà@b¡…vL
@BLƂ/ñ?¶ ß´*·?‰0QxåçG?θÐV<<@Ee*§¿çIpŒZ¿áoáÐêê¿çÞl²[¿á['§åŒ·¿ç;ØÞ¨íJ¿ØÖ^¤ÑAGNbll3FGL J0145.6+8600WN B0140.0+8546?ïª)mò»¹?ßå­/¨4?UøÍÛPç?IV.‡¯B‹?'¶ŠáU§ž??ªW=-;?ï±G¼È?'i»'¢º?Bêâ¿<?U¹qIk#ô?'Še
Š?€üÀ*ˆs?ï äzK/?~Vú¡ýëü?i^˜A?6?TÍäÏŽB?˜·²Õ²(?{Œí?%?ïVK>¹Ø?r¥ž¡G?l1Œ=ØÛ6?Sÿϖј"?ˆž
 ÛS¯?pGâhäð4FGL J0151.4-3607?닫†oßüÀR™—_,¶AÀ:Õ,D,À<Â(äû—»@ʆXõµ@ü\Wë‰?Áú"³Ùa?°ÔâšêQ˜?ïœÙŸÄ @ AO€›Ç¿»,€¼}õ#¿Ü|؃9Zë¿é§¢pØ°¿ÚDí$±W¿ê>ku™à¿ïô¸~Œ"
AGNbcu3FGL J0151.0-3609PMN J0151-3605?ïJzÅáº?Š¼¬òlí?kÓûwõ
?`£ "45Z?"6'âù¿W?‰S À^Ò¯?ïq¡Lôt?"ÁÇuÂâC?Pàˆ/ÔòZ?`I£|Í?½Íނ¢]?'ïÿäŒ=þ?î´gñ?£Â…‹­?"ÄlO«†¼?w'Ÿ¸R'(?ªÃžs=Y?ŠBâ_ڙ?ï>Œ»É?ç*¶Á¾°?}ÛºÄ
÷?j³ÌæÑ®?—T?·ƒð?~Þ¯€\¯4FGL J0151.7+5455?íþÔq[âÕÀÀJÕÀ:{93'uÀ<)'(±Ïñ@x97Úû@ßçžà*x?Îû"áN?ÎgΛYa?ñ"ÒTÌ
/@ô"µÜÆ?¿¾HyìU(Q¿»äqY3¢ð¿ä&&À^)¿çO[½•ø$¿î,¦AÕÏ?Ø_`'÷–¥AGNbcu7C 0148+5439?àÙ²äòʱ?ÅÅÙTŒ?'¾[°É¿_?Š'­¯Ÿx?Ý ´{
Ω?ÄùhB¡­S?æ¨É>³Q?ÇˁK?hk4+©¢K?|[…©a9?Ò}—k+F?nj¬¼Ø`?ê{§3XÖ?§ÂÿV3•¬?¢Ì6Çænð?'
­PªðÎ?Ã3±9ë?¢Õ›\%æÓ?^¬²=?‡OïusFÖ?xú\Ø"8?cl¿©¿Ì?¤tþyÉ°?†S½zï[4FGL J0152.2+3714¿ßeÉ»þÒÀ8Sü–ÿÀ:¶ÁȌÌÀ<†xºüÀ°@‡r¨¾û@e%îÇÉ?»üžw?³£çÑ5Z?ñ¯Nìő@ކÀùÚÍ?ïBUåæ¿ãã/áD¿æ³û¢n¿áêP (êZ¿æ:D4w¿ïÏöbreùAGNbcu3FGL J0152.2+3707B2 0149+37?ï=¡IQì?lO–=n"?V\¶ÊÌh?N×ÿÚoÎx?–æzoUå?ŽxÂ1+?ï…	àY¼?…'i§æP­?A(ߣy«?L€ýàæ€h?ªùÿ1öS?"óløŽÿ?ï$¹ôIìY?W—Eø?fÉí'gÙ±?S"
ºé?˜ƒÆuyÎ?|ܦN"ë€?ï)êuìÕ?v	¡•07?nC@ëïP?U—Ÿ}Ž0?–úI$çzÖ?t…ö)',4FGL J0152.2+2206¿îo[»p6§ÀCM¶¡è´À9²j²üA/À<7Üýœxq@Üωë|@åO±;?¶Y 
ý?¾µ9³*q@+ÞàˇR@[Õ¿É¿³Û÷žBÜÛ¿æOâ+ã	¿èÞÙ	1µ¿ç'Á†¿ïÿùµc#¼?êL»P£‡AGNfsrq3FGL J0151.6+2205PKS 0149+21?ïí;"2ªÜ?wTMPAæ¿?HXvü"$1?YÊçûiË?Y\œ`3'?q+Šò>×6?î¡ÞrÆ'?©ÉÁՅ¯-?pî»*¾J?€Ù4ËsÕ?£ÄVü8¿-?§¨—Æ?ï7«E|J?~MŽE»?pJS¨'Èö?cý¹Oœ?"øfZÄa?z1Çefuþ?ïm–HÉß;?|F\NˆUÝ?rƒy]
^€?eŸ'Ë#?‹X±>?vEÌ«Çh×4FGL J0152.6+0147¿i‡X˜UHrÀLÅM@$³>À9mRj0'À<tBÇü@%L=gµ?ÿñ|D=?¯Çˆ"9¿ƒgáfÝ?Ôi,"AC@	B1}Ñ?¬¬j_Lõ/?¸I*ì<ԝ¿ár]ëm¡Ä¿Ü"í*¿à¢¸'¬eN¿ÓVPn­\ÅAGNbll3FGL J0152.6+0148PMN J0152+0146?ï¿A›–¬T?w)Zøá?Cœ¢vw=?=°_
¨S"?}ë°À[}?uڌxÃ;?ïÐeLÔ²–?(™‡ú?(Xæ"Ñ?A­¸5~Lv?w
"}	€?}×
a}J?ï‡iÔ£?ƒP¡—T}?hsÓªƒ¥?`ƒqØ!f?›]dJöNÊ?'L¢Mþ†»?ï{ g[?spÑp#?[–fð'àô?GQyx¢?Å-+­
?r!*c¢4FGL J0153.0+7517?Õ-Pèr<*@)É%x_.À9û)=+ÇÀ<L"4­†¶@ TB…Þ?ÿ&ò³c%?·—MŽÿä?±BZÃpÆ?øln¾#¼ž@$ìH`¿èK·ùÖñ¿­Wåš#,¿Öþqàm¨¿à(l/Ô¿à{'{üP¿áÍ´ôhó	AGNbll3FGL J0152.8+75171RXS J015308.4+751756?î0VóFó?¤"ÑÆ~ ?pTÊpÖ(z?e=´}ƒ?ªï÷}v	Î?£fiU`Ô?íÜØ㣀?­£àmÑú?!†2ûJŸ?‡8ãh(Æí?®[a«f^¤?ªs- v©?ì¡Zù`¤?žØ¹'í¦H?Œùν%‰Q?~3Xiç†?·UõˆI³?›·…iS0h?ëZ¨âN?›0먿Œ'?¢\ãՎ?‰ãäŽÇTç?»ü¸{¤È2?šw'Îfg4FGL J0153.4+7114¿ä]+ŠzöI@!ò!ȧ¤À:jfóT À<O$V ž@!"U©€Â?þuêMT?º$ëFàd.¿'y(_ð€†?Ú©=;äó@:šþsì¿ïûÔ¢.=«?ïÿIŒ;F¿è€§?tŠ¿Õrü øH&¿Ü­ÏÜv¸ï¿ß{"¶
nAGNrdg3FGL J0153.4+7114TXS 0149+710?îMð²HÛ¸?¡¶{¼Eà?V6%,+s+?S4¿Hai?ªoC²èæ?¡zötöò?ë
5èdzî?Äzð[Ÿ?aLJì3?u-ÔE6š¿?Å÷4Ùy?ÄM:@Ñì?ê;Ӂˆø_?£•ÕُÖ;?†v_t~Ð?p‹¡ˆ_?Å©L֖?¢Å¼ô ü\?íŽùâ?˜å:*‰8?‰i֏÷Á?{ ‹åêï÷?´Meœý?™2æëFz84FGL J0153.5-5107¿Ç"V)¾{ŒÀO¢sÿ¬*À:Ìg¼§»›À<z9ŠeI@üÖ~|\È@
goF	?ô¹©š¿¯"èÁu?áèæ€Äa@øªgr*?ïøs^œm‰¿éú÷k¿éQÃA2Ð7¿îݼ¾â©X¿ïý®aQԉ?ì!1¾iÕAGNfsrqPKS 0152-513?ïïeØLL?‡Fc{Ė?TÑ%bå6~?†'³)
c?HÆT	übß?Y1º1+?ï@ãYl?¢
í\*WÌ?n)5Wû´?‡b—;
—X?"zŽ1S?›ðæë·þ?íd·>H;c?˜¸ö¨ÿ{?ƒáÏmW_‡?® &ò÷?²^ 8û?—*¬ÀÜR?ïÍçSã0¾?'Ê"Ìì‡?*zG6—àô?L_ZÍHf?x8ƒÔ²á€?'`¦<.&P4FGL J0153.9+0823¿êï<ÏÐH"ÀI°·ÃPLIÀ8ðÑn=À;ª¾®&@7ÕÞCl¼?ý%'6¥®{?¬ÐZ¿6?´s"·e•@Jñ£EêÆ@BíPøì¿Ðmâ;sôn¿ÕŽ_©³Ã¿àlâiø¿Õ¥^~~¾¿â1úï,¿éäÞq9þÿAGNbll3FGL J0154.0+0824GB6 J0154+0823?ïњ8aÁý?nòbý}Ñ?4ÞmÁ ù'?,óË ž¹!?uäüóñë?nAÿí&?ïžWÂ|'?ˆg¸Vþ\½??µïœÝ|ý?RüÔè
LÑ?‡l_äQ(?‡4ßQ[æ?îù|	éö™?ˆºes.w?sI'&»àÔ?k43ë ?›þ4ù4[?…þÐcî¸?îzQXTß,?´k)>?_c¿/ʬ!?NåüºOÝ­?§_́3·×?ŽÔsúÀ4FGL J0154.3-0236?ïì¾£OŒÀNž¢×/ýÀ:ݤÌӂÉÀ<œ¿eÛüë@| ®vJŠ@É2¼î¥?¼´ßWD5¿©P>Ü´¡?ð¯¢ðZp@Åôw‹§¾?ïíYx0=¿åföyn€ç¿äìÔ	0'¿â!ÛA¯¢Å¿Ö3~݀¤*¿ïÿî,˜å?AGNbcuTXS 0151-028?ïà
Kƒª?e©§(?@«ÌV%?5Ÿ"514?kÒI‰hÔÆ?c",&:È.? Ò¯ö?‹s«P"K?:GØCy*Ù?PúuAf?ŠY	89/?Š­i›$¶?î2õVô"?A°JÇC?s	hê™ÝÅ?`/
Fƒq?ª~ƒ={	?'߸¦ãì?îÆÑt2Jª?ˆ,ÂÖî®?cr"
'?UH]Ñ×jË?¢[Ɯ¬O?ˆ+IajŒ4FGL J0155.0+4433¿í´Çn$\À0Ú©÷µ®£À:b-—è¿rÀ<C8d@…"†?þ]Ã_eÁ%?Á ¨A'<°?Ós k°R@"¡ô±î@žWˆ
€?ïù$¯ñ¦¿ÓÄÐo½¿ÛÖ}»Áã¿ç2BÝË!Ò¿æ\¤¡	¥p¿Ü9G'RAGNbll3FGL J0154.9+4433GB6 J0154+4433?æh÷x#T?¿+ô27ў?¶.*s"k??®'\0Çá?ËEå¯Å?º˜_2'†%?ìsÿ9‹·f?µ?ŽÖìŠS?¡"ѹ*U?©@–šÇ?³W
A?­¼i,Žëp?âE»ö%'`?µîÅÙ"œ?Ðâ'R¬Þ?³Ïõ¢‹}Ä?Å$÷"Ä`¿?¦Ü³"§ãb?êü9X"ý?ž¶Ó1Ê? Ñzë>Ò?‰ù¿U{»ê?¿¶`¿œo
?™@j!Ü4FGL J0155.4-0625?ÓÉù?5dÀP`,'À:óÀƒé.,À<–'Jÿ†@r)0zò@>
í(Œç?̇œ–ú?̇DÒ»?÷¾XzëX©?ÿúa÷ì¶?ïþ\AIvl¿Þâ˜[V¿ç·y^:ÈÔ¿í¾I¡ßŽE¿ÕÀŽeˆðÕ¿ïÿ5jE8AGNbcuPMN J0155-0621?ïeQ¨,©?˜iÜ° ?oOšS¨&?rš‰)IQÄ?˜IbŠOõ½?–ŸGÝá?î»B¶¢E?©ÛD[˵Ž?x>Qù@?"]1 1 -?¡D
V³­?£‡jÕ¹!ý?ì‹Þ¯C >?™Á9»©‡?›%*jœ<ó?Ž»#ì"\Þ?´×¿ë;îË?"ù©|=?íëùó^B?'Ã̏¦L?'\XEÉF™?vÇðóÝß?¬¶êOWÊJ?''tÚRŽÌ4FGL J0156.1+1502?æÆÈNÁa½ÀF€.#)À;›ªgG6öÀ<Æ´!Û@!w©úå¹Ù?úk³\¹>{?ÕT¤òé?ÊÑ(¼Œ¸¶?ööc3«þ÷@gÙ¦¤ð¿é'æ!1¨ï¿ð?ð¿ÒŠ…¼¿Ü8Ʊ•¿Þϑ7ËHhAGNbcuRX J0156.0+1502?ï¢#Íû)?ƒÐswT$ð?A
L´V?7mæ"ç?†eØgµõ"?ƒxEPÄÀ?ïA0ª8?"|èaîŽv?LÇíæ`?\­f›K¢?–ó²( 0U?"yf	?í¤½¬0_?–ŒOZÀ
?qÒåˆwæA?bO¯QµÉF?±Âkºþ?•…§ð•?îk&¿üŸ,?'W‹fŒ?BKÅj?@N7±*?©7Ÿù?'=»@D'š4FGL J0156.5+3914¿É™\]pÀ5èÍJ¡À9ÒU݂&¶À<djQ­q¾@áaKI{@wí"Ó8ø?²jËOõ?šµÉƒŸºÎ?äBÎFIm@…䀝Ÿ8?…Ñ1½¿â'Ÿ¿ùTÀ¿çÿF!!Ä¿åHùn‡Q¿ä_ÞÝpˆÿ¿æyi"ƒb¡AGNbcu3FGL J0156.3+3913MG4 J015630+3913?ïۖvéä®?pÀ¿PÜ{?:›A'Àýì?1_¦cäf?p‹qñ˜k?pbWW¢a…?ïÛ+çâ2?vÔ¤ðÞe?#:ÙTô?:U~y»?¬?qі7?v*ڃò?ï8@$.S9?}æ¤>­³w?fm¼Ã×?P|Ri¬?–*CáÅ^?|/ža°I?ïî	LÜ?Jë[~ÃV"?3'·˜'Ì?!É.¶ýÊ?]ý(-@;…?I#ÅÜÇ4FGL J0156.6-1758¿íäs˜Ó÷ÀRÓo~=À;NÞÚ‹À<łw>$ÿ@Cl§s!
@EÜ@W?ÅøvHܒ¾¿«—s#¹¹?ã̤ˆàä²@9˜¸=S?ï8ßî°L¿êˆH8}õÏ¿áÊDAxpT¿ÙGőo(­¿â"^~»qܿﱺ!Ï]¡AGNbcuPMN J0156-1800?ï[Pâ2â#?Ši4'›Oa?Zò™´Àt?Q´øeÇú?'íäo¿?‰OÄ£­œd?ïz#v}?æ¹˜sN?IÄD(Euž?^:l#dð?Ž…4ôž	N?Ü¡ö×bP?î
ïqª›?ßÒõ`r?wíäx‹Ó?hmîÕÙ?¬QdyâDØ?\¡€†Mù?îßc0¨?‡šË¶xh¥?\€/©†?QL{[Æí¾?¡%Í_©b?‡7@ì¶4FGL J0156.8-4744?ánšÊ=½ÀPp@ ÇÀ:mDù.T§À<ªfÄZ7"@ŠÃvˆr@Õ~œ¾H?¸´XaÀå8¿›ûÚ'ö7?âa0œýç@	i°|ʬ¿è6úhŠ'¿ãe—=$¿æ
5bhß¿Ý2GZ²~¿Ýw¼Ú¼N¥¿êNHÝêVvAGNbll3FGL J0156.9-47422MASS J01564603-4744174?ïèeFܑ?`hO}†-?;¬5‡m?1®é±lÿ?d7ƒœ¾3?^›Û€ƒ"?ïÜécX?wæ4‡@"	?!Lzïn?@þhXÖ8€?q؞ûÝ?võK	Jm?ïKÛ*ˆ?y©v;Õ?bHn$Ék?VíSšVØ?"T¶Ùç¶?wCÒé'Ü?ïܾ]®¨ ?[rÞüvt¥?6âŽ~'ˆ&?*K«%Ûäê?p2¨@‡Ã?ZŒhÉï"4FGL J0156.9-5301?ëqÙX˜¿ÌÀN°å^³À9Ü¡|¼êÀ<³†ª©Œ@¡ 47?øת@°Ê8?´->§…–?º¶¢Êê@F"Ú8+@‰qü­Æ¿ïáâ"Ÿg9?í…ʬk-?¥G´t'Ln¿ÖŠš"U•¿â3EaÞí6¿ÂèÛùe‡AGNbll3FGL J0157.0-53011RXS J015658.6-530208?ïùu<»?Jjï¿^ÿ]?#'‡çÈ"?$Ö/Êb‰2?Fɉ•Œ?F÷ÜãÎ?ïÙ=¦îÄ?xԒ_bu? h^Ɛ4?4S'A€ó?rü<'iT?ws=ËÑlQ?îñ¥rtZ®?‰ö•ñ0yU?iëûAUu?^]'Èo8N?žÒIIû¼?‰#Åôß?ﲪüÌà?oú[û.¾&?62Àšô|?/7ðòÊ
?'£ªÈ$$;?oÀàg!4FGL J0156.9+4648¿éua‡ô‡À--"n)ÔÀ:ë<©Ôz@À<h-æÃ@Ÿñ‹¡´?ÿ–îú>¯?Ðy<¬Ù'?՞9¾g¯@Xä1ò@þíï]'?ìç`vã6?ï­Ù¢H>Þ¿Öl|ªöc¿çˆD§Ï½B¿âtÒ9ô¿ðAGNbcuMG4 J015651+4648?ï¶-óö?¢Ã×xéo?zÐ~GåwÙ?qÉÔ]}Ê?•Õ H#x?¢†²˜±?î]4é‹Ú?§"†¼9©?yÔALžÊU?†·Åß)2?¦ò)=®…è?¤ª¦,뗓?ëסѬô? IÎͪ?¦·÷±Ä?'m¦±ì9í?¶:·5v¿x?•÷zÉ¥T\?ì5ä\=Z?Ÿòø1Rį?˜^\_&gg?ŠÔЍÃÏ?¸9F"{]?›>ŽÉŠ£Þ4FGL J0157.7-4614¿ì.ç|¯ÀP´˜5‹'À:LvѵÀ<!4x­Ç@ˆW+µæV@ê}ík¨Æ?¿à	ëf?û?ÌꗸîÉw@–l£—I]@A	—ÙP?ïü=¿ÿ	¿Û==ÛWÕ¿åÒ¾^"¿èÛ¾WîÔ¿íþ˜ ó–¿ïÿþR€ÖTAGNfsrq3FGL J0157.9-4615PMN J0157-4614?ûo=?…%ð<æŠf?sÒW/"–?}-`–R¼t?{e«P¬Í[?yN'U°Y?ï§ø–qñ?'K#1Òù7?K&M•­og?nwÀá)8?"OuŸH­
?[åP–¾_?ìôîsÊ? R|ýè?£_ώ¢M?'³)Z1ì?­ž¹¼l?"‡ŒRÿ?ïC's¯|è?~v!Ûzª?Z""¦°n¬?N—Øá ?•øè?¥\-?}Ée–å4FGL J0158.5-3932?Õá uù"ãÀQÕQ֌i/À9‰'TPº-À<L~D©}<@îJ µ'-@LQj‹?®p®hß?®¬ˆ×[@Gjdø¨@ÝÍM{2ü?íŽ:‹I¿Ý—Ä{Dš¿áž¾fØ|-¿ãâC çU¿á^û}å3 ¿âaÈýŠYáAGNbll3FGL J0158.6-3931PMN J0158-3932?ï+Ç~'±?«úí*ŒH?G
'ÇŸ¾?jÑCì?‡Díw2ÙÂ?ªP¾©Ë?ïÏÕËÞ¥›?€Q[4³™Ê?)ö6Ä¡]ü?C÷o{êb?wEhZˆ' ?µÐ	@?ï öšYz?'p'+¤"?n±"Æà ?iÙaÓ?ƒ"?˜eÁøX?€^ùÜ›?ï¸ÜO3\­?fwc¶-«?Píá@ø²)?B¬ÍHÛñª?V`}??dɌ]"Ù4FGL J0158.8+0101?±=^O«ÀLÁ¥~ª*À:MŒuĨ;À<W#I±$@.û%OÅ»@d¤Ú¦?µ3>ñ­V濱*óÄa?úõ³;?ï™"/¢&}¿ã·M>w4¿ßêvjG¿éI­=ef6¿âò|Ÿ7é%¿áa¢
×I¿èËRä©bdAGNfsrq3FGL J0158.6+0102GB6 J0158+0101?í¹'­Þ9?°'['¡D?‡DAÛ#?šrΑ'AÇ?®œÄÞ%½?¬‹	ì©F?íÈä¶ürè?³&˜"ªA?‹AðNþ¦?ŸKîôL$§?¬¡o%í?°_gzjòÝ?ìšã´ˆ+?žb¦¯™?'Ùº®d?ƒšÁsvÄ?¶âqc°%¤?š˜ÉWº?êÿ+(T7?§bÔÚ8Ù?¢ÝÑ£;Ö?"XêK"?¾˜é=ëÀ`?£vôµ-©o4FGL J0159.3-4523?è˜WèÒÅhÀPÒt>–=ÅÀ;ûAT^&À<ZÁ#>@ƒ+̱º@ñÀoz?ÃïÊhC‹E¿­Ähœ˜ôÐ?çM}å-@
·y
²ñ?ïÆ­czù›¿ëϚ!~ÕÉ¿ââ΁WÙ[¿æÿ¢!¨qN¿á¬Yûð¿ïÿýç!éAGNbcuPMN J0159-4515?ïó"|?]è-ÅDÛö?0uÃ~Ÿ?+ø4"ÐÉ?TбÀ0?\@Лžz1?ï¬Øz¹Oþ?‡»4½"‡'??9"'-·?Rêbà¡Ñƒ?ƒÐ='¢?†TÖH©<??îÎ!ҟQÀ?Šµ'®Ý?jô9šz?eˆÀiìüÞ?¡|@öÇJb?Šc¹¡\è?ï¨þ"Êo?ozøÑH"?:jå487?3'ñðþ¦?"í¥˜ˆ?n°™剸4FGL J0159.5+1046¿Ý"ÃM¿réÀHSπÜ3rÀ99I—"ÇÀ;ù'ì®@¹O"ðB?ÿa,:=é?­ÊÞW†? ¥ ÛN½?ó(᠙h@Aàz~¡F¿ÝèÀž@Gn¿Ý/ò6ᄿà†=~搿áüŽ''Û¿Úª-e"؏¿ÛLáD¨ücAGNbll3FGL J0159.4+1046RX J0159.5+1047?ïÅÙªeŽ®?u°~!k\ª?8³šÁƒ*?/øÜIí\º?{‡ñ!@?u
¢&$?ï¶o7Ks|?ƒ´BUï?/Ñîsøâ?EÈ{£¶?ç¶åiQC?ƒ/afUÚ?ïTSåPÔ?'¬;ô å?iåR"µ%?_Z²¾¶
?šUÙNÈ?€Ûu¬ò?ï`(ÜË?y'ˆÎ~Ñ?Ps±Y8??Á^S?ùu?'ú,†Û?xã61#m4FGL J0159.7-2740?áÌÔã¹pÀRµ;Ÿ_À:"z-ëÀ<ÍÄC'O@È÷C«@
¨_/:€?·iŸUñ#?±]CRAf?÷Ê	ÞÒ@È7Zµ-I?ï÷"_mλ¿Ú]&š¯™¿àÁÞây|¿àÂÞZ"Ê¿ââ½ÏÚ¿æÑT¼÷"AGNbll3FGL J0159.8-2741PMN J0159-2739?ïu®ÕKž?ÏGÔ¡5?WƍÉvm?J»y£Ûv!?›yÓé¯?~xWä°?|$ÿ?Ÿ˜·¿7?L)x÷sÎ?_EY4úPŽ?Š'	gI
-?ŒØæ$…?íèTEKëZ?"	Kœ5?€]O¢`ÒR?tìgr¼ÊÈ?­cg©Ó?P!	ý™@?ïå D¦W?|טF¾ê'?s# F¶6Æ?_Åuý#ð?˜zs彧Q?z72"í0'4FGL J0200.3-4109¿Í3\è}MÀQ"Ó0"'À:‡4–àµÀ<'oQÇrñ@ p6åDgä?úéQgÑ q?ÁblÇ(ž?Áۛǜ6W@)ý¢W®=?õA÷˜(«¿ïÌ7Z?åéáæ9…]?£ûüÞпښr¦æ‰¿ßGH~sùL¿âÒ*AGNbll3FGL J0200.3-41081RXS J020021.0-410936?ï[(1¶;?‡)l¡,Ç?_Ç'[¦C?[××ߗ»?'ž‡ës~?†³ê œU?îJbZ" ?¨¶s?fSÌB?Šv"LYt?¤`Íí¹?¤Qˆ<§q?íê7öåj?ñçm(¢)?}®ˆœØ­'?p¿JÒÎñ?­©klö"š?Ž×‰†3б?êi(Q/U?¤'½+eŸ?–ϗ"³ó?…šð9?ÚfÖì0?£U¸ËA4FGL J0200.6-6637¿í¥Mܤ'´ÀHŠÎóÀ:#8ê,YÀ<…6žË2@@zž×œ	@ÐeÁ•?³î`¬ßX?'dmÆ_¨æ?ÙiôE6ÀÜ@pXËô
¿ám‹zÖ¿ä'z¡†Î¿çúVÞ3&ž¿äUûŸž¿é±Èd¿ïú3¢Ä»†AGNfsrq3FGL J0200.9-6635PMN J0201-6638?ïè×ÁÍb?m^dî;]4?Cgÿ¼p"…?[ºl—5Ñ?bN>CàyÂ?b:t8À^?ï»á§ÓØ ?…¨Rm©ªO?4-V_ç?SRö¸?€g<¢ßE?"ª4"u=?ïIúθ&9?|À¶áŸ?fU)-1£?Vˆ(lt?"ö'¾?{Q¹(Ÿ¨Õ?ïäº&bí?Wýýë2'?DcøC÷?4'®'áž4?fBØ{±?U'h6C4FGL J0201.1+0036?ïr݊+´ÜÀLÌڐî¢À;~eæä¦À<ÆCnÙÒ@!4՞'?ý4¥ùú-?Ñ"×ü?®-žÁ0?ßŐÃ\5¶@‹ìé͹‡¿ïL³'#i?ít來
 ?ÞF}¯y¿Øá<O¼¿Ýü"C¿‹¿àqS>ìNóAGNbllMS 0158.5+0019?ïë´v&Ê?ftöiD?!È¡!–?% •1¿¡s?cÞÁy×&?ex·»¦Äî?ïÀ] nAM?"È4ëÇ["?3‹¨þ-bl?Pa'ÚÐ?~˜u8üƒ	?ƒåÛE]z?îni[M!C?ˆ«
=†f?kÜ­¶¤VÑ?U¨ÿ‡lÁè?§[Ÿoæc?‡–R²µ×î?ïs™7†h?|,½OoB¤?Dª¼À©}{?=5{Ý¿E?çƒ)-¢?{áˀ"«Þ4FGL J0201.1-4347¿î—šë)ÀQóà7ÝÀ;­†)zLÍÀ<ïÈN¸Ê·@!ñҕ¹?úÞ@'—?ÑV€[¯ÿ?ÇZHJòlš?÷žçf¬"@4•¥RÝ?âÖtì;'?ÎR	!¼¾7?åǂ«@‹¿ãæxw¿¥™ÑÞë™}¿å²?'ÌÎAGNbcuGALEXASC J020110.83-434654.8?îݛæ†!­?—Ã_cK'?dò.0b=?ZgÔpd•? ×´—ÁM?—­Ôs?ï†å8œAß?''6y$?KÍ?8q¦?bPR¯÷?Œ‰Ýåhm´?>áä_yÎ?ís§xëz?"ð~Á?~p'Σ<?rªÕì
‹?²{»~pr?'L¢£|#õ?îŽx¯
˜ì?"ða‹£ê?F…N"0Ðà?Gç|K†ºy?¦¾_ÕE­î?"É[ܧS4FGL J0202.4+0849?ïvOÖ4³ÀI0ߛÜjÀ:Ðè¨ËeÄÀ<tíSUª@ õ.vŠö¿?ú'4Û©ß?ËÏö¸X¡'?̸Ž;íkÿ@H&	@Êúmnî?é¥C†g®¿êâàíB¿º¤›?áíE¿Êü¬äOx¿Þ1¯$›?â¿çJ¼¤¡5AGNfsrq3FGL J0202.3+0851TXS 0159+085?ïppƒd°p?†ìKÂÌ?R܄«L˵?O×ÎåbL?Ä'Hµ%E?…¸o&ãJò?ï9›ïEo?"i"ÐÍ?S׳Óþ—2?a£ÚsýWu?—#ä×hÜ?'c£¬´É¾?íœs™}O§?"¼
=š?y<
í²±ï?i—Šô	?±ˆ¢…:W¢?'qŠ–d7Œ?칗é€5þ?–à¿ÃÿÊÔ?oeZƒ?^ónðÉ¡Ù?¹;%‰-³ï?–²´½m
]4FGL J0202.6-0258¿áâïÅ0‡nÀN9a€M˜9À:sëLÔÉÀ<cݯs²@7súž@óI¾ó(?¿L͹ð…?œÒ¡^E@ã?ÜðqA¶®¨@À¿aKæ?ïóÒà¿ç1e}³4¿ä͇§ÿê¿Þ¹%˜b¿ïÿÍ?¹Ss?ïøŸƒ¾fAGNfsrqWISE J020239.94-030207.9?ï5ѐ?'NÒ0Ù'?m#·fæ°?e³hðQƒü?•£º—ñ2?f§µøm?ïA¯ÅÑ«^?–\aù쯌?]5'ÁßgW?p($¨|øT?•ö¯¬ý?"r–ûŸúœ?í"/y'ç?"Jƒ˜ƒË›?‹á˜-?%nùo?¯ÔÎÒcU?°û»èu?î·rn÷ô?ŠKZ1ûÙ,?vQyVþ?g\8bþk?¡¸®áUüÑ?ˆ?."4FGL J0202.7+4204?År"‰d9³À2ÞD""N×À:¿í½qæÀ<ŠÊ'_éu@ŸøUӍ@ª‰žyÓ+?ÅJ¢Ô€Ë?·ßT"@X?òΝ‡dä@M>ê¡t¿éæÓ^6l#?îß¦Ä$ˆ¿ædèÕ.›¿ØÚf}ãZ®¿å¨Ñl×Å¿ïþÖj€˜AGNbll3FGL J0202.5+4206B3 0159+418?ïô_sŒ!?MóG<"¿?#9ø
Fe?¿˜S"o‹?TÙÙæ
/?Lªôͺ€?ïÕ¿Ò¿»(?xÏ$âh¶þ?&xÀ(}é?;u,üât?tlPŸ©)/?xs3Ӊ=?ï#Ql&¾?~‡Ì"ë0¸?eb"Å?UÎ¶"5#?˜òæ:¥^?|'}âÍr?ï­z€7½1?f5Ž§V†?Wƞ"¤YA?D¿'Ësº?¨Œœ)?erßL;ý4FGL J0202.9-0225¿ì/¾µ)dÀM÷Õ<ÝÖàÀ:Ó¡ÏɏÀ<|%ä–.@ ÈAÒt>?þŒÇÄOOÉ?ÄÊàä[ߥ?AB g"×?þp'Ldë¿ïïê^-1ç?ïá¢!¨¿à:r•;¿Û907Ö0#¿ê—Š@
\$?ÙTÎäT'õAGNbcu3FGL J0203.1-0227RX J0202.9-0223?ï·O*Q?}AÌþ¸e?CËwqÚ?Aö.tea?€ï}ô†ý?|Z…¸rD~?ï|}›ôV?1"ç6n?J€íc¦–?^µÞ¹¢K?WÂÑ`j?Žô—9W¬?í'+½À?–rG--•¸?†ûŠTs¦?€"Í/]?°5ì c†?"s6r\Š0?íT˜ëQ?š¡ixüp?}C
""2ã?p¯‰ÛO¼•?³‡~|4X?™æAN$ۆ4FGL J0203.6+7233¿ìÈ@">Á@$ä$=Ìê)À9ÛtÄÍúÊÀ;Ü|©žÊ[@iŠ·( ³@@Tƒæ?½Û"zÿ$¹?¬`áZàK?ðô:æ…Û@0aV݁?íh"ÿ‰;¿ØŒö=^…F¿ã¸j¤ ¿ã¼]ž–®ƒ¿á…òB}(¿èRçcQ0AGNbll3FGL J0204.0+7234S5 0159+723?îˆ'5™ÍÁ? 
¾˜ÁÅq?bƒØÇÛ?Y‰¬ýPš¡?¦UOåsŠ?ŸšªÞ'¶?í›yýÜ?º´L˜Ä"
?dÛ>¦ÿ?€ÖÇ^uSn?·F5]##à?ºaB8û–H?í¹uì·4?›È…¢ ­û?'ñÏً¼?t¡©rmT?´óúm?ñ?™~û@Ôø?ì
S—'?˜Xäñ¨c,?ƒò"ÌáŒí?lzµÏÙµÄ?½/—Ì?˜ƒ¶1 Ã4FGL J0203.7+3042¿êòPW0h~À=£gŽÀ8—'¡}"À;°-,ˆõ@z<c3@ )»»,'?£N O´Q?¹9@}ôwŒ@¹Wɱ@š³ÿʥ¹ãf_¿Ý¶µÅIK¿ã½ÊÁ.Þæ¿ââ!LÖÈ¿éy"ù÷¨¿è²#3
ïGAGNbll3FGL J0203.6+3043NVSS J020344+304238?ïEùWì­?…=ƒGÚß?XMÏÚvm?[µÕSӉP?+Wð	…›?ƒ¾@D©2?ïij¯ä4­?€›e:7¸Ü?4öÇU?QQ×OaÚq?|](¡tÉÛ?cÒ¯ÇÜ?ï(7Mð?‰hãrBL?©.ÇÛÎ?cþ9@#?"ÊÝ«K	?ž%ƒÌú?ïá—uTsî?[4p]Dz?+õe˜#ï4?!;KŠ˜?l©4R	ÒÏ?Z"LäòÛË4FGL J0204.0-3334?â-}5N°+ÀREQ.ƼèÀ;1ºÌð;À<Ïïå։@ ŽÙw*.?û­ L;Aõ?Ó5šìð{?Á61u?ðßn	È֞@Œ_Ó¥."?ïK°¢ÊšÃ¿é÷3þŠ4!¿×c.qÊH¿Öž*¢ëÒÌ¿à$>adŸ¿èý?[_¢AGNbll1RXS J020413.6-333345?ïf‰'/i?½þОzÔ?'¸ççhð?¾Nã›ó6?ˆ´ÍSä?ƒXjÕl?ï Ã0A<?‰æã01?? °&¼àò?Q´&D3?†Ö.~yÉÂ?ˆÈÍdad?î#‹¼"?‹íd}£`?nŽ
Éù¥?W[¾Ë5‡'?«Þmœœ?Š²»ÝòO%?ï&‹zU?|PÔN3a?E,–l?:‰½i£?›s_€Ð?|%Ò¶‰`4FGL J0204.1-2919?Öð[å%€ÀRuæFñVÀ;«*ÏÀÀ<÷P²ŸúÝ@¾žÆ)D?ôÎ3Ÿi½3?âUÝLvÑ?èõ €"Ž@V–8@[ul=ÀÖ¿ÒÞÎWˆ?åõ•äsx¿B­­ê‰v¿Ô1‰$i¢¿ç©$@üõ_¿ïü5ĊßAGNbcuPMN J0204-2923?ï/³›<<?—ˆ¿ô?{Ê^CƍJ?wÌ7Ýa©?"õŠÕx?"Å®é_(€?ï>ðÍ´'X?L
;'ø?iœ4ó«?ƒ²;Qõ Ú?•2Â햫?˜ìYï
?í§çj?œÐŽ\Ž|Î?•qF‡7?†Ð¸*Ú?².oCžÀ?˜´3ƒ¶ š?îšC¯úJ½?§ûWv"—?^y½Þ§Û?]~庺!Ž?¥g÷fd?~
-‹ÀP4FGL J0204.3-3140?æIfÑEWxÀRa	éÍ³À;nÈÏJ«À<á4s¥J@&ky˞@d‰Ø[?ÈÐæ¿'æÜjl?ÊîVŠPPz@˽€~•‡¿èòÁS¿ØÔ¹*X™¿å!s¸^€¿¿ä´_î}!¿Îüâ~ºÆ¿å2R˜SH|AGNbcuMRSS 414-035156?ù‰·÷?~yÆ=»:?J*ÁWÀæÐ?@+ˆO?Œ²Õˆô-?}·² ""?ï¦k=Âxf?ˆ:'$&º?;*ˆ'+h?NàÞ?EY?…‹ÜN(J?‡S6´w'?íø¤.æ	?£T]D€?x<­ÜÖ ?j¬L\­d"?­n'cÖÛ}?ŽÔˆ¥»5?ïwGBX?{Pg|ì*?@
<2ϊÞ?:­]ë?–ÊÖ'˜©?{R²·ü4FGL J0204.3+2417?à{YïrÀAÔdE#öÀ;8é
55À<¦²ò03¤@ ãóÏ/?ù)p;Ò>&?×µZÀ?ö?Ô
ª]·U?ÿ"!bPW@®A·/£?ïÎ3i¹×þ¿ÒÙxÛ^¿æ†00Is翶Ҫ¡¬¿Ñ¢#ᆘ5¿ïÿ® A§AGNbll3FGL J0204.2+2420B2 0201+24?ïpdó.Mh?ŽXÝå­ùs?Vå4ˆ;Ü?Q¹ÌµŒš?…XÝÏ?-ۙŽà?ï\&³W?'0>ÛRà»?Gå^§UÁ}?b¶Af?"»þŸåN?'FǼîÐx?íØ^Gzý?•Š2}cÑR?}Š©ð>à¾?r×ËLFÉ?®Íô݀t?"y¶,½™[?î‡K~¢?Žlö1o,¬?Pwc±ç?›?NËz]ül?§
 *†¤ç?ŽÌ3¬–ˆ4FGL J0204.8+1513¿î¯ºç¶ÌÊÀFŸÂ¨†œÀ9Q/¯ðóôÀ<0rÅð9¹@Œe¨%x‹@ª?Ú
£?­ÚÉ呿±?µ=+Y m@ä¢üïªG@ûû˒æ?~Ãvˆr€¿ä"¢A]îH¿ã(Ÿ[zz¿är_îÓ¿êl5恿ïüÑaÜéÐAGNbcu3FGL J0205.0+15104C +15.05?ïØD8Cä*?häÿߗ?Bµí» %?6܀=§'?qœÍ V†Ó?fÝz‰
—?ïªäô½Ý?…†î†÷Œ?6>—?I'Þ[¶²?""Ò¡°_?"›Hg˜1_?ïž•X&?†Ý¼€é?wz'4iÀö?t[µGäÜì?—­ˆÇä‹?3Ùþ­Ò?ïÂRkÖº?gúÏÚ$?U¨)\øÔ?EiîÄ5Á?yŒL…}dë?dzz¥Ká4FGL J0205.0-1700¿éêwwÛ®½ÀQŒí"1{À8ôh§‰FeÀ<DÕòæ<@Ò}'Þ[@ƒ&ùz«?¨x'¼›?´ç<t$•@XxœÉÏÂ@Ôo{bø¿×¬| 9›Ø¿ä¸MžïCð¿èpžmhä¿éŠÃæ¿ïýò߆õ¿ì"ñÉÜW"AGNfsrq3FGL J0205.2-1700PKS 0202-17?ïùè`?<ûìÑ+â·?%le™À5?ԏ@PÜ?BáRŠø%?90•ËB×à?ïĄ¾2û?'dÓ£_Œ?E3ÝÚÉî?u¨@,ÎPö?{%+^DÆ?‰vÃÅìm¦?ï+wÓ?d8")œ^?s™ì´½T¦?iüÒ»tŠ¾?•¸µòvH?}·²÷?ïð*M
;?O<"*»&®?<U¢qïí?8ŸŸ{oj?X–#ÂínË?HßHÂ)J%4FGL J0205.2+3212¿çÍûÃQÆÀ<†Â&€À9#T˜Þ‰À<
qÉp÷º@\b}x¦°@kÛñ,þ?«°
ÏK'?²)­ß‡ö•@S¤!²Ø/@<¥Á›p¿ÊuIRk¿åò•ž¸<r¿èTS¿DÎç¿èQ°''¾¿ì1Û¿ÙÊ6¿ácA&
AGNfsrq3FGL J0204.8+3212B2 0202+31?ïâ\Üe(D?z¯¢Ê)?<™]A¾?3—¯ÜÊ?j÷÷˜H?yü—"m²?ïÊá÷bó?{äáµàh?)…"4ù^?:ªaÙ¤%ë?yÂ×µ=7?{;¡òöÿ?ï!3t?"s,¶"?q•;Ò?bó›ßÓa?—™M×퉄?ò¡}™e'?ïî²MޞŒ?P(œ?¬â?:±´;º	?-Fku·$?[ê·Õ³÷f?M¦¦l½D4FGL J0206.0-0958¿êzáV,î‡ÀP[2 f<uÀ;ˆv{‡_ÛÀ<ÊXÓÖ¬@!Tÿ™Ó¦0?üámÙ!næ?Ðrñd0×
?•ñ{ؾr—?Çn,ÙQëZ@%v\'É¿áî=•ŒÄŸ¿ìäÚEÀ¿Û̘ÊfÀÿ¿¸4ûï¯P¿ãŒÛE5"7¿à!4-.6tAGNfsrq2MASS J02061590-0957174?ï éxµ3?~ø.¥kk»?0ŽÛÐ|?%€_E)à?‡A*õÒLñ?~w4À?>aµ?Š†î°Fc?<óÍóf˜¥?Qc½­<ª?‡Ñ±ÀÌ]è?‰x®±ŠNi?îX¿f|?ŽX‰ýdS?jå¿è@?\-¬(©z?­j«ù9¸?O±…TÑä?îÊ¢/Oð?Œ…i¿Â…?9œq"™H?2V-è(¯?£#×t(»Ú?Œ‹®@'?54FGL J0206.4-1151?îiàS'NLÀP­[[ÕÀ8üQo^]À<(.Ï÷#¸@mO–U¨@TdÏ?¥
¸À¦N?¦'ÎI#µg?ýUúX R†@P+ÁÏâ¿Ò×Gd˜…ó¿ãlh'î¿åÞûmÊö¿ãPPzkÖé¿é={Uá³å¿ïÿ3òuÓÂAGNfsrq3FGL J0206.4-1150PMN J0206-1150?ïÛ+Ÿ9ž&?©H{'8?i9¨G½?©Q È\ü?W5pþ¢9:?MÀÕZb­¦?ïÔÁ…™ÎO?C	nʓ?,ŠÁ¿oj?P—àV˜"?tºç%]x?|ð#ƒ¦*?ïO0ýýjq?{:MøÎÈ?g	pµ´Õ?X󇜉Ê?"8¼Ò;ûq?xåÕ	³E:?ïøÆì"u?=ȓÀÄÂ7?'œ²h
ɨ?äÝEÜó÷?I©·³ê·n?:ËF<é¯á4FGL J0206.8-5744¿ÖOF¥¼ù¬ÀLP64êÀ:ÌÁTɅðÀ<ÅZã{dû@·´Œº?ülA÷ò…?Í7xý—ÅÚ?ÆæÇ	i`A?úÀÇ¯;@ÿ¥' T?ïÿüÚ±'Þ¿êM"M1â¿ÖKž¤pb>¿Û¥i±t'¿àé"89,q¿ê"]u&ÊAGNbcuSUMSS J020640-574948?ï"x=ç?†Äfù¢`?FmÝ$†Äå?BøÁ2}?‰ÙϨ²?…VOœß€©?ïŽAÍÇɶ?ˆM°v›d?Aýì;Cén?RÛR{đ©?‹O­ÊYSØ?‡Uƒ|勉?íõtj¿?"™Ãm¨1`?r.±>®)¤?iŠËáf?®bé¶sŽá?"Ç'YYöá?ï(º×lÏ?xœáÀ&eØ?T2\Q÷ÀØ?Cxé?÷°?™¥™Ÿòê!?x\qu_4FGL J0207.4-3855¿ïê†;mê>ÀQòº`À: r̦6`À<´zˆ\Zt@5ôå?_@Œ|½ÀÀO?¼J^¼?¾g:vÉ`?ôšøÄ¢[à?üòUû_1i¿äÐG«<#¿ÛnÂÊ £¿åÇ]Œ£¿ëÒ ;I?fßހ(A¿ïÿõ¹U ÄAGNbcu3FGL J0207.9-3846PKS 0205-391?îìU[Ä=Ø?˜åçí[p?cTêÞqQ?a¶'X·úA? [›ž;R?˜'ú0®M4?ï=ž¡=<Š?š•,büå?_ûI…Z²?qâÓ%4?–LwFà%?—±yX4û?í1¡5¸Ù?–•ôSÊ?Æ¸ÿñb9?€¨/R]£?²º2A\ù?"Jl]ÊÂB?ïpoðê?‰"D#Gtp?bWÚÈm?_™¹À['‡?œÑQ–¨Õ?ˆˆz >º4FGL J0207.5-1049¿ºˆˆ@®=ÀPr½f'|À;^ìz>À<—6>@!¯vz° @êE%£þw?ɲN¨Ú¿ƒdZ¦gr?¼ 
|xˆ@ã9ÇÝû¿å™‹¢
+}?îñŸoÇc¿é‰Êï|û¿íJU^×&?ã_Nyà–®¿ïúÛ2ÁlAGNbcuPMN J0207-1047?ï±èq&y–?"r7li[9?W ¥,»?n'ÿCz¿?€¡ãŒôó?Æ·Iý?ﴑ0,C?‹Ý5ê2:?>aÐJö9Š?\¾½^ó¯?è¥y=¯?‰ÅÔ»–¹?í†EW°¨?•÷š}@i??';¡óÂTä?wæ‡ÚjÞ?±†ax?"½"ï݊?串GY$'?y˜ýš7?LlÇ£;?#Ä×/6Bƒ?†¢P(¬?y~3#44FGL J0207.5-2402?î®î·Ð‰ÀR$œM©?À:F´ -œñÀ<•S–€	¦@̓P:@FúZ¤'D?·¦53h2?Dd!×Z?ã€e`WÆ@*'Bðë?ìpÐL´
¹¿ÞJp¼€¤U¿âŒ
¿Ü$¿æC$Aþ¨¿Ô³œzª¿ðAGNbcuNVSS J020733-240202?ïñ¦¦?TÜÿZ½·?,¡™îÜ(»?&€³¡Úýæ?Zg§tØbÃ?ST°(N‰‰?ïܐ^(Ç?xØÍæB%ý?ŒŒhš!?/Kë³¥:{?q_S¹úg?xtŽ;^?ï.ð‹G—?'^8g³àX?jÅíÎÒ=œ?`ðˆ€†§ê?™ád4¼Åb?|¶nP?ïèÝwÆM?R§å?'êá+Žµ³?r
aÀ?e£Ú&úŠ?Q•wS˧›4FGL J0207.9+2203?ã²*
PÍÀB¹v_Ø­¬À:ýîðäJÀ<‰iêe;@AhÃbì@5ëÄߘ?ÊθŠJœ0?ÊRøJ~ÿ:@
Vz`o?ÿ2]šåÉô?ÔÚ³àl¼Â¿ÔÜõ8ü¡¿Ëe*§µ¿étËNG‹°¿ÌiýIÂ@Ø¿ïÿ€éŸkkAGNbcuNVSS J020801+220241?íÔönu"?¥îÊÿ×`S?{óŒœaº?w)pHãî#?¯@ÍDž!"?¥.R˜ju?î.hç$xC?¢—8ÙŒ.?rºàDž6?yµÒw:‹­?ªÂ‹‹5?¡N½Oî:?íBÖcÏ®:?"®=Î\OØ?׳$]?'-–W"º=?±æ‰+•Å?Ç‡.Áxô?ë_V»vø? oÄr$_²?ƒì¯£Pç?x©ÃªÍ`x?ÁCãÇ)êŒ? `üöcàü4FGL J0207.9+0953?Ê!ÚóMŒrÀHL	¢@1HÀ;U&£øÀ<a"ÌÐþ‹@ƒÌ_"?ü³^f½¤?Ü~9¡ŒW<?ïû¤$èî@›Ç;"T@¢°çiR?ÒËA&»×¿Ó"2ëƍ¿Ø{{vmð¿è  ‰wãf¿é¸âό¿ïüÒÿ@èSAGNbcuGALEXASC J020754.55+095014.0?èÕ
¦(l?ÎÀm>‡M? «1ÜÑeD?›À³SjÇ?ȁð+Œÿ?Ã7L¿3ß@?ê#¶ËpV¡?Âõrè%?¬ºw³º‹$?´¤LTì_q?ÀB†åP¶?¼K°Ð'øÆ?éÐQ½‹ â?ªœô­2?°;~¹ûbv?˜Aõ±9àö?À ù¬ÓË@?¤A+@˜Ï€?â~r<`´?¶%é¯c¨?©Àl¬PÂ? {¸Õ¦¦¿?×Ë
öÇ´?µ­'î¹Ór4FGL J0208.3-6838¿é¯@4x'žÀGyÂôÀ:oî'B³À<£ˆÁÛC@F¶š[`y@uIÞpc??¶ØrGp,¿£=Fÿ».?îó^ÂC|@¼3Æ«öh?ï0hå¿¿æNèÑQ­¿ç|>¿ÙI]¿äÁgÿBÀÅ¿Í
­B˜ÖÑ¿èÿ[_¢'AGNbll3FGL J0208.0-6838PKS 0206-688?ïH;
m$?´ÐŽƒóD?aP+·5Ë?S¼ŽÈl»?"Λy;tÀ?)Q²Â?K?ï{dÝÆ!‡?ÇOš
-9?D¬á~Äp?^Ž»$ÏQ'?äíÀ_±ö?Bú:?î¿3ŸM=?‹'£z^¯Ð?kÜ=Ð^£ö?`EÉ3$™?¢O
iB?‰û¹µò%?$"Ô?s¤
¹.è?V'Ç­µ'?L±]…8Uæ?ŒBT´›?sepÁ"ì4FGL J0208.5-0046¿á¦oÎ͋—ÀLæ…3±tÀ:™ôàèÄÀ<Ã¥Üû@œ=n€@§¬Y¾O?ÀD
Ý)¿~ÀŽ–—m?Á™ÁÕ?þ¶E|â¿ãÑx=Sr™¿âDr@bï¿ål"ABÀ¿Ú5…=A)¿ì4"|+ʉ¿ïÿý±q&´AGNbllPKS 0205-010?îïÝ¥ª$Ï?­ÉùcXáä?s÷JáÒw?†…ŠSßâí?BxñŒ?¨®ãŒqÙ4?ïkžXÃI?'ÕÃïÓ{?Oû´Õvì?a8Tæ?'Œ`Ž;æy?'Çôü‡s'?íà;M•?'ÔŒ\üýc?ˆTd	?køÉ;V¤?«ç5Zæ¥?áCE߇?­M?‹¢®‡3KQ?~>ÿÌaÞ÷?m–*}rÊ+?¢?Å5^ò³?ˆ"·A¢»4FGL J0208.6+3523¿ÙÙ©‡µÀ8ÞT´:çÀ:¢zˆ\ZtÀ<|î¡2ë@ ¬í†««??üä17°pv?Ãìmçd'È?·ÛCÝûH`?önõ›øïk@7Áe¤8?ÑÏ3"f×z¿ßSȟ@¢‡¿ÞµÿÆÜ¿Ñ	žD#E¿áÎW±—½!¿Øµ€ëLê"AGNbll3FGL J0208.6+3522MS 0205.7+3509?î÷…1>}"?ñbÒâIŽ?T¬"ÏNbð?E×1w?ºN?ŸÄ—«;g"?¤tAów"?ïѓJA¦?"ÆԅÏûc?\0CV¶?g‡=¶³j?œ¢ÉeVuÙ?"¶ÁôŒ`?íàÉëòä?'¡Úñ"?t_^ή@Ò?`"3LPâ?¯s‡‡k	¤?Šô¦1¢?ìg^'±?'Hßҋ2?€ÚJ"MOô?hm‡?5?%?¹Ù{·aÀ?'Dö:4FGL J0209.3+4449?ß;7™…‰À/À¯¸kÀ:r™A…ŽÀ<|á®ai@ fŽ›ê'?ü€0ŒÅÛ?Äò™åﳂ?»!²,b‰?önøÜP@@[Èµ¿ÈE»K¿ç³l|*¿Òf'åK†¿ß§üaåοà••_x6¿Ñ,Ó}kÃAGNbll3FGL J0209.5+44491RXS J020917.6+444951?ï[×n=²ì?D,+Ô{?CtÕÑÖü-?9sç•ÂãÝ?"ék‰ºêŒ?9Ì
!ˆ?ï'[Lý!?ŠØÛLç•?=¥˜æ'ŒP?OàW*W'è?Š»ÿù"cw?Šd'ãvT?îb)ÞAõŽ?'B‡d#f"?mÑÔª"6?cåЈHo‡?¨Q–è? QcO.?îÐC1°?[ÒUGˆè?^mfÖÖÎ`?JfáQÓ?¢P˜ö.w?[ØÕ\é54FGL J0209.3-5228¿Ó¾ˆƒi"üÀNb$‡wÀ8—ú…l»ëÀ;º•µßJ~@cŽy*
p?üêzAå}ž?¢î½¾h?žFøaûó?øù5
£Çñ@ Àžìå?Þ5ëŸJÞv¿ÐOõ
ÙwÖ¿âi%]‡›¿Ó­vÛ©‰|¿àKm̌¿ÖG EDØ¢AGNbll3FGL J0209.4-5229PMN J0209-5229?ïÃUіa¥?¨Ò²9Ä9Â?>7©ÃŒ½?lq?v¬Ëç?|qœ˜—5<?§ÍA)Ñs?ïÐFZ´Ô?€ÆÎa`h?'šÒ@"Z?=>
6Z?wü_ õM?vCVÄ@–?î㶯IÚ?‰µÄö+uº?m"ºݏ?hæK!}6z?ŸÖ'Æ[Ï?‡Ü•Ÿ¸¶?ï•6?ÖU?róU†—ð0?I—‡™Eí«?;7Ôz{mØ?‰÷ê˸?rEŸäÅLæ4FGL J0209.9+7229¿ïü-\|@%àŠï³À:ZÄq´xÀ;ïËWÇ@[ZÈ£r`@›ß>¿Xp?ÀºAYç|ü?Ñr»´K¢@í¬«ÅH@;OŒZA¿åå¥ `r±¿Ý§4ø/Q&¿à½¥6Ü¿àŠ#opÑ#¿étNáºo¨¿ïÿ¤àõx¾AGNbllS5 0205+722?îüèÚÅÂC?›ýÎ)™P?"f~¦ŒM?'{R"`?ˆ¶üQBW?Šƒj…?ï^Íp.š•?™÷_UƒÀ?P¬1ÎùC¤?b6ϵ¿$?"ŽÝ=?™.ê)OG?èh£½d"?®V…2¼à??»\5˜'#'?£½bÊòÀv?ÁüB¤ÁÝæ?¤×S2ïš?îX×wr×D?hŸ±•?eá	®Éë¥?Yщ¿!ؼ?©wíåí?'
cø4FGL J0210.1+2518?ïþZ'-û¢ÀAWÿ›V2À:ã쮤"À<_ˆü"d@ 6Ä÷@hÑ?ýéXÎG ?Èív{†'?ÂèSX?úþ³†ªª@ †ó¤§ë¿ïŸr÷na?ïD1Rˆc¿½"ëYÕ´R¿Ú`χã¿Þ»S'Å@ç¿éþý×0ÓÝAGNbcuGB6 J0210+2517?ïËRH‹"Ü?tƒ"dl?C÷ˆàP~^?@¤Ò
@'7?w×êž,A?s>-é?ïWOYÀÁ¿?MŠUéä^?J¹°´îüˆ?Už:Ù™?"@GB@P>?Auxѳ?îR	2"ó?Á€¿|Ò?rF—w£^:?eîRÍ ©D?¨–œMãE
?‹îϱ'L?îŠCuù(ý?ˆÕÐY<8?xŽ–ن?gã?.ßG ?¤Iõܬµ
?‡¼¢»4FGL J0210.5-1445?æ<CŠÛ7ÀPõ!…Æ~À;0|ý À<®6Ýß@Š
D·)@í¤Ûìû@?ÉøǼ톬?–C<j¿fˆ?Ê:ÜúA@S>"u¿ç`
¹(*¿åõ–àVÂZ¿äÅêà´
^¿ç²PIÄo0¿ÂªÍ‰
UC¿ïü¨AÓ	'AGNbcuPKS 0207-149?ï™Þ£B
?€R!M֐?W7	éêyó?TÙ´JnzÖ?†¡uòB®?¶Ðq€
™?ï¡0½†Z­?Š%OavŠ{?;"<Ÿ"ó?Q.X\Šˆ?†Ú¾¹lµ'?ˆì}Eà=^?î €œí?Ž£ «Ó·?yÎòˆM4?fe³Õ›Æ?ªÅé¥-…Q?Œ؇©ª?ï«ü	 ¦?p.
íOo?/›ÚÜKL?)^'Ã
Üÿ?"'Ž/£ee?p	¢&T´²4FGL J0210.7-5101?îô8÷m_ÀNã
ⴖÀ7Žî&¹¨-À;"Ë7¡W@ª¢%.b¿@é¾?kOÚ?"yy»n?µÒÿTÿ6@!þÃüC²Ý@7hÿóÀ­¿Ï'X&`¿áûúëÄ	¿ä¶U⊤3¿å桇N¾¿êÕ#³co;¿ïÿÈ¢› ÛAGNFSRQ3FGL J0210.7-5101PKS 0208-512?ïÈÝ@ç?rö-Þb?Y&bäߏ+?Z>XÙàې?uGÞ¾§¨W?nBÓégüm?ïcó{@¼J?šÔ8eê~Z?XYws©$?r½¡cÿoò?'ûù<.?™tÈïLæ?îÛ
Vvw?•EÎÀË?'[æMf?/›	óÕ÷?'A¸=ä0È?†ÝiZá?ïì£k†7à?Vb\Wñ#?=ÐD©Î8î?7q¶bp¡?_EÉ°Ü?Tiî ©q4FGL J0211.1-0646?ïŽrünG~ÀO.œË}AÀ:­ß1S_À<œÂ?«º@bWšÆ•P@ˁ½?ÁÛק·?úàe8?ÝÃn_E°@Õÿ¾^Ë¿â<Þ1;¿ç窟ѿÐ?Þ½:3¿áólß&k¥¿â;‡•‹¿ßPå€wߋAGNbll3FGL J0211.2-0649NVSS J021109-064551?ïÝÔd:?fìiO£Þ?9¶*bü-Á?-ô­ÉXƒ¤?oÈfO@?fEí-î?ï¼ßÀ&ÎC?'»äÙ?1¥»`•n?IR-PTª?€:âLj[?Ô³Üéå?îÊñc}Ӟ?ˆ'HÅJÓ?m,îù¬3?aó
nÉÕ?¡~؇þ?†¬L‹§Ñ?ï±Ñ´Ð ?hK'«Œ³ù?@)ٞ[–?1P¾Ð"Î"?'ˆõ2E0?gõ׉±4FGL J0211.2+1051¿Ë¬L®ïJÀG¯Š	ÞÀ7³´&ÚÀ;FÀh Ó@ìœf}t@hG,{Ä?—œM9Tñ…?ªÑÆþùè@¾×@Än@çuK[ž?Á]GXÚ¿Ý×Êâfçì¿âÿp"§Êµ¿àúLÍ8,—¿äÀD=Njſä.¢<ÖAGNBLL3FGL J0211.2+1051MG1 J021114+1051?ï')ÿ}¦?™Æ\~–?AÀ<ç2'½?8ÊÝlpF?ŠY|nmsÔ?#-lÒlX?ï"
…›QT?‹ƒå((?Dl´÷
W+?R}±$L'[?‰µÓIºÕ'?ŠöÓamdÓ?ïøü²7†?‹—	9j´á?t»ßÉÿ–?qI ­×ý«?–Ñ褆o?‰kÊó›É¬?ï³­»ÏÞ?nþ{91¸?C¨}~‰BÇ?9,¡: ,?Ú	`ãtM?nVn'ô_4FGL J0212.2-2559?î‡cÑቝÀQú¢‡~äâÀ:þŒjÜí¬À<·†«€L@´Û%«
Z?ý#·ÊÝ"?ÉÈ#š¹Õ#?½.ëÐÉÃ?òðñõ{AÀ@¤ýÒ(V`¿Á‡
`V,¿êHº–i?­¦ŠÃ½Úl¿ã¤ÁëÈ:—¿ÞáAäP÷ê¿ÖޏØO·ÎAGNbcuPMN J0212-2558?ï'F™3³?'¯&…Ç?@`'%»?5þ‹Ñ
ûù?Še€­5°ß?É¡jµ\?ï">"­¸?¾–eX‡2?B°Z-5#?U¸s ‹D?‰ÅZV1¾Š?ŽOãç·Xç?î/®µ8Å´?‹&)xX'ª?q<ÈËpºé?]8'Ïr$¿?ªÝ{"i?‰rT\?ïä	q#?&q̝{?HÉ@«ÁÝñ??¸cŸw•7?œý4ùsÌÃ?õùü4FGL J0212.2-0219?âGÛ`ZÖÀMDÁ~ºñÀ:åG5H·)À<£zm"h@:iàCw#@ƒýP"WC?Á·ýO0À¿š6°¸'xÛ?ÕÚSÑä@…ѳ'gq?ïçu$oK¿â#Ê|"¿ãÍug‹*¿åPâÁ*Ø¿Ü•ƒŸÝ*"¿×¶ %#ûÞAGNbcuRX J0212.3-0222?ï¨&ŽKL±?|ŠÓ1§W#?H/Yˆ/:¯??û¹IÎ?"sfÔ©à+?{ù'ž(6?ï´V¡£ùÛ?ƒÂMºeC?3,ÙàbñÊ?Fé·±"<«?'PðÇþqä?ƒ/ª)Șe?î‡
ÿɱ?Œ+÷è'??qúƼJ‰.?c#ZŠtûè?¥OÎHzÎ?ŠOhéž=?ï"9P"Þ?r9´ç4Åÿ?GûL¸d—?9$©²wq%?q÷-7Aþ?r*†yY½¾4FGL J0212.4-3502¿ê4xm­‹ÀQ¾¹¡vÝ­À:Wõ ¨ìôÀ<«©f–7@j¶JU @3T¦J'?¹ÒœÅsE?ƒA©ÝMg?ÉÖ§.ë{@ƒC¹=N?ÑEœš*
¿æ·½ ‡_¿Ù`ÈWG¿ÞAàËy¿å³2'#ƒ"¿Ê	 :2*õAGNbll3FGL J0212.8-3504RBS 0292?ïUºÁ!qÚ?‹o2¡üO"?TÅKÀ^}Ù?FßÐn—Â?"üSËÜì?ŠºFÅeF?ï¤û…Ñö?‰ØyèÌ7?6úÔǑ?Ißéû'ŽŠ?†F0/êÄO?ˆ?Üüà­?îU
¿·Ÿ?:U<ÓG?uðÆoÚÊô?jmûÄ6(?§ñ;Aé,²?ŒF‡¹"–?ïc!x¥`½?tÀ
o•œ?U;n$v?CáiÚY¥?'Ha§I?sêUՊ'L4FGL J0212.8-2721?—ež·³—ÀQû†ìë¯À:Ìb¯!ÁÀ<·îŠŒ¶\@2œ"uÃQ@CTc.£?Áö
HX^f?¨Dͺ]‰s?ä鋧i@#f•á(N?ïµÖ±R¿×s×}ªÐ¤¿ãZŸ2ਿé·?Ò}涿Ì=$ä
d¿ïÿÿÊPËAGNbcu3FGL J0213.1-2720PMN J0212-2719?ïhÅéß)È?ŠœÖÌoöz?U®Yà4p?Q•¡ó~OA?'Œ]&€
?‰Ñ{­ˆ¤ ?¾Ÿ?Œ 
d"æ?@ýÃTxºß?S`‡'È:?‰ª´jÈ̜?Šïó;ë
¨?í¯A1ŸS?'ÖØå¢	=?…,&ž¨?uˆ¥"®v®?¯Àãm•c;?Žà–[†ªR?(—ßì?qœ«Vý-†?R,oì?HÙ,KÓ¦]?Š–sÌ·?q	dAo©p4FGL J0212.9+2244¿Öˆžl´&ÀB/ü~k?êÀ9ÐK¨ñÀ<<µ…ˆj@ð2¸9?ÿäçUO?µó8ò9î¹?¾·]¤ËÑÐ@
/»¯n@õÆžh5¿îÑҀ@M?ïæ#J‡ã¿àËÂFa
¿à¥0 Y;Û¿ä<zo1ç¿ä÷ƒŸ‡DWAGNbll3FGL J0213.0+2245MG3 J021252+2246?ïíP¿òTt?UË¥g·]?D}Ì©ÙP?>›Ž'¯!~?[ZÁ5,v?RO¶@©?ï'wܱ°J?"î%Ú{6?I-ý¢¶™?Wr'sYÄÄ?Ï8"¹Áä?ŽÏDT'¤?ï+ÛøÖ?~Õiڈ_L?j©ñ"¤æÏ?[aSX`³?—Hf\¢Å?{f«Aê(?ï% ·B5/?{."'7¹?v;•£bލ?a¼`IH²?•Í®à¢ž?x­ì…W4FGL J0213.8-6949¿ç"±/Y×.ÀFÔ×ðí=†À;!ö'õ;À<Àµ™ª`'@"5Wâ¿þ2?øáv<?A?ɂý5uWÆ?¶.Ý8)è?î'gbÂ*@ÞÇÌÿ¿ï³ «Ü'=?ïõf4€¿áÁçâÒɿ؀Q~Í»_?€>—•]tпârá锄AGNbcu2MASS J02135882-6951360?ïÀ3%#e{?w·ûZarJ?5µÚ -?/Ť͞‰?~•'«@‰?wFäó\bñ?ï¯þcÌ]?''?"Ñý?+aùÂz4e?B7ìܜ?ƒ'ß%ÞՈ?Ÿ1e°…­?íçï(æc?•tg??b¸ˆ½¶N0?QM÷8
Ä?°*Âyk|?•4V£)"?ï"‡õ¾–8?"(¡Åp­?Bä4¿!'?@ÙªÞ[‡œ?›ߢ4,h?"vð¢4FGL J0214.1-4733?ïÇrøÅùõÀOù
¿cíÀ;€£n.²À<ê»ð¶ù@ qâ;žè?ü#æt=¿~?ÝΟ C×Æ?·_Kêå?Þ±]û³À@ßyw»#¿ä¾¡@W%¿ËâäfF…ö¿ã[ºÜ	€²¿ÍÍâK ¿ÛV,\\׿ïó±"L["AGNbcu2MASS J02140989-4732357?ïÜMޞë?•Y}xwËë?)=;ÀÝ*I?Röœ†¬-?q&҃J?"XU»M¼?ï»ì‰òFu?"æJ{¶š¿?+ªÀðñ½ç?C8ƒh0©?€–2ª›j?"'Kc^?îR÷óñë?Œ{+CßÑ?pLja ?`s´@ßÐò?¨ÍM#•?‹ZXà?ï"m¨úŸb?tgc\¢¦?'ó#Gch?)šS@Wð?ŠÄÉ4:›{?tvBßz"g4FGL J0214.2-7025¿ÜÝ&bP"RÀF[ÕìlÀ:)?—Å"À<vׇ:òD@Å´Júz@Ñí@	ÛK?¹g'Ñ_Ú?°¤žìzù?ðB'!¬øò@?q¯ðž¿Ü€'q^çí¿ç@D"­Ç¿è'&ëý¼¿èéé¾4ú¿íA8D,¿œµÐ±Þ´×AGNbcuPMN J0214-7027?îɸ?NC?›ÅÕZ\®?w®û"9H.?pŸ2 ç? nœš—bÒ?šb‡ºÃÙr?î&~vF÷X?¬¬Zm"?~Q"`W½?'M"µsó?©ÍôOŸŽ?¨S"sà(?ì‹Ë>_Ý?Õˆ¹‡?™yäa¿:?ŠÆ0.3|?µC-õ9Ã?˜g"›Vµ?îñBý°H^?ˆíÕ!ö_3?‰hFàØÓx?|3'n¯?•#|يŠj?€š©\œ4FGL J0214.3+5145¿é0ó;ˆÀ"s2&ÄÀ9÷kÅJøLÀ<C:8
2‰@ ›ú©ÿÃD@ñ›¹.Š?®CµâO•ê¿´'HnXÎ"@7E«I@ÑZÚôã?ïã)›üå¿æ™Sù|X¿ã«xßdÔì¿Ô±qÝ=r¿âkí>\\!¿ÏÑß[DÊAGNbll3FGL J0214.4+5143TXS 0210+515?æuЗȭ?Á{}'Ȇa?i!g
ä-?t+"	øA??҉Å66Î?ÁTÙ¾…‡?âI-ä\¸?Êóº²Ë5?ƒ^^V¹Ãj?§d;"üA?ÚÒ±DÁæ?ʂ!´l)º?êÅ(}¡ù?¥ÕâK×Ã?ŒÔù^[Ÿä?vÀËÛ??ÅכÈ#¾?¤Ïçö¹?éE¹Pú?¥½¨Vûã•?¡E•E`I?‰Ô«û S¢?ÅyƒÉguØ?¦˜; 4FGL J0214.4-5822?à眄¹hÀKÇߏG0@À;}ÂO›HÆÀ<òÿ4(%¹@\E*¯}?þû˜\'·Ö?ÓG÷›,–·?Ԙ\bq?ýëWfï"b@
ôù
†¿ïQ¶
éh?ïÞ'bEo¿Ü—û3èe¿âÎcûR¿æU.enâ¿ïÿü¥¬¨AGNbcu3FGL J0214.7-5823PMN J0214-5822?ïæþß5¤?‡u`"Ü¡§?DZÑ-É?Uã0Š¦Ã?d­J?…³otfå?ï¯>"amþ?…	M>i–?8G2q:¡?O,ÆÜ@ȇ?ƒn!T&i?":ÿøÉßÇ?íϽ%¨)S?•ÅeÊÍ©.?µÌs	W,?"_ÿIk°?ª©Gkø¿4?'ö'—¢?ï¸eëàŽ?i]ѹ?Iä3˜Ù?:¨G¢¼Ë?€HAÖ¡Žæ?hu\úUV4FGL J0214.6-4333?×xÕñ°ÿ3ÀP Ž4À;ïiÃèø|À<ü]¿Î·‰@"Ù¾9a«?÷ Â'Æï=?ÚrÁ`'?²Ì)cы£?×"ªú¿ú+?üøÃñ11?ï¨HSUèj?ØãŸAyG¿êcnÏÁsÓ¿ÉÕ	‡=K¿Ðu¬¿ç<¿Ç""7ª¼,AGNbcu1RXS J021439.0-433319?î꨾êw?œ§¯A"
U?B	h—Z‡?<Ý*€ªt?¡
së¶29?œ‡HÙ£ ?ïj©ŠËäá?–ù¹M¡?N&è†:#?góÚ]ˆu
?'¹·?1õ?•£–á"h!?팣øzXY?•ÿ™'ñÈU?o ¨'Û?ZÔZ#'?²¡ß¦ì°Ÿ?•"¤Iÿß?ìàj(x³?§ÏŋY¿£?XRnâ—+8?ZÍ®§pˆ4?¸ºó1ݶ?§ßOá˜4FGL J0214.8-6150¿áj`û‡94ÀJN(ܘëÀ;6¬7+xÀ<ÄR)˜¾@Pþ39é@ˆwîN&Õ?Ð|³úîÉ!?Ð>͛(åÒ?öýã¼Ó[?î—õøó¤Û?ìŸÝJÉQî¿Ìôœ_ÄW¿å`¿'țæ¿ç[`m~¿ïÿ Êƒ+?ïôìp×±AGNbcuPKS 0212-620?îûqÄ°h?™Õqežç?wû%cµ/÷?xó†3?š'þ¤?—|ò€«;?êsiI·?ÆW³ù—?²žä¶aþÍ?¼èz"q?¼uÿPI0?·ÙsÿŒÁ?ë[×àë(?¢§Í8KC?¦Ð©€À/>?"Ô!¾†Õ…?¹¸ì8F§?š!f¤S?æÏ`¤Ìß?°/ˆF(?·VœÙ~A?¤¯VÌùÖ?Éu!Œ
]?¬*|šH°4FGL J0214.9-3722¿ï@lüq¥ÀQip£×
=À:Ç	á*QãÀ<¡ jْ®@»ˆçÕ@S3¹jð9?ÇàáÂ'W]?±>lwL"?äq|^ö/@¹U¹ÅÞò¿°ˆUà˜lÚ¿èæÙóü¼¿èyÞp¹&¿ïÿ·äkO?ïîÑk%¿ïáûÓJ•PAGNbcuPMN J0214-3729?ï󄛧˜–?eLÉïÜKó?7ÛÁÕ½-?A`]´¬…?SÑÀYd£?bêuw?ï9
'‡Ò?˜Ö]KŸÿ?VC²³G£?yÉ÷ÜbH¡?‰éGõ2?"³–›uÀ?íoǐL{Á?"]L´½?ÎÊÁv4?uœ#ÉQ`k?²Gê%m_Ò?'ÝÌý¡º?ïè
u[ÿw?b™½YJ×?ÂÈêÚ?5ìØTN?g™˜à("?bƒ"H?64FGL J0215.3+7555¿çå=ð..o@+ÈÂ?«ºÀ;)A® 9À<˜?gôÛà@"cÑeõ?û!DˆÆ¿?ËlØÆU9m?ÀDc²,
?õ#|ÜÊpÒ@'ÇœŒ=;¿ïÿîͨ"ß¿ïüúAzÓ?ïÿÿ^ðP`?y7»ûe³Û¿å&Õ!/$±¿k7¯çUAGNbcuWN B0210.3+7540?ï'n%]£µ?ƒ2ìÏ!­?5äòb·_W?.}P _Z?ŠµOWä?ƒw·<ïå?íãªLÛä?µWêëá+?hÒÎ>"uŠ?{éîW1
‹?°'/ËÄ?´ãE;xâ?í3;ʟÒ?œÍ¯nC¡Y?tŠ+ýöÐÞ?aÉÑ«G°º?µKa˔Y?›ÍžÉ´r?ì;?sÓry?¢OŒ–pþ$?r&ÏSµ?lҟò'g?½¢"o:©?¢:/	6'4FGL J0215.9+0300¿ïäeh±ÀJÏO'õfÀ:Ÿµ<OÀ<wRœ…e@›	³Ýè~?üðÏÆ|P³?ÍJ‹¼[?ÄØOø:ä­?ø¨Øœ
è @)_SL®.?ïþdŸfã¿èK7 }£ð¿Þߤ¬ó¿Ò¤^Ƃ;¿ævîÿ|¢h¿ç,Sæ1!áAGNbcu3FGL J0216.0+0300PMN J0215+0300?ï?pUY?'"ÎÅ:?A§]g6î?:jw%EÆD?‹ŸzMwHE?',ôd¸?ïTä"P"­?'QhÖ1Rô?Lˆ=R'5Ì?Xh2]P¸?"+«Y¶?'™Ý9°k?î!	õG?'ôPÿ:V?pí·U«>?d›â$x?«Ñ©ÀÒ§ž?'Ù g–³?î裈>?‹ŸP.†þ?gô…¼ºCš?VçSe…
œ?®B-k°z¯?‹+ê|4¾84FGL J0216.5+2313¿ìXügçgÀAÍ®_ú;›À:'{&ÁÀ<deÀN9I@ º¦'Ço?û)—Ãք?ōK±?Ç@÷Ií@Z	`ÑÑï@=*WíR¿·²Ãa>3¿ê‡/3Ê1è¿Øì]Ù¤÷¿ÒHj|öu¾¿à¹Ã_eÁ¿âsè/(âwAGNbllRBS 0298?î¹K]nñ?¢†&~|Tð?{í¬•ƒ¢}?t%£q†Œ·?¬Vµ·xœœ?¡oÄûØe?íÿ\75°?«×ˆŠ§ùÞ?p·e]Ô?|@XP`Aâ?­ð(OéYA?ª)Šê.?í;@ÅùÐ?˜0P¾‹§Ä?'0_ö¾Òÿ?t`¢ŽùMœ?³ßó
øW$?–X´Â?ȝ?é‹Ó˜‡´c?¡y¦1¿?'I¹C>â¾?r•I_tX@?Ȭ	­@G? êò&á\24FGL J0216.6-1015?à1ˆŽ.sÀO䦰)(À9¯'OH<°À<Sû!sî@´¹¯ä‰­@ÑÿÁìžú?²"¡9öñ¹?¶"^—&@rá& %9@/«$ÜX[?ïØ~>õ3¿á[CÝOÒ¿â(ey×\s¿à峃O«9¿æN'b™R¿êdüAGNbcu3FGL J0216.6-1019PMN J0216-1017?ïèÖR&º?p}Å`ƒ?,K¢¤"0¼?*1¯Ÿ5A?ed󯯸?o³Þ/Zw?ïÙϲOd?{š&¡ú'‰?&H‹z1úy?Då®órþ?reâ||'ý?z"²(y>?ïB
A¤^ˆ?zú·¼í0?gúŒ…|q?[·JU~.Š?"¿f:пY?wýc8åÊ?ïà–²¬¬g?V7)´/g7?<ùØw**?.2
Vm"?kÊDnSu?TѦ)¸d4FGL J0216.8-6635?УCf‡ÀH2â\
WÀ9ßæÆsxÀ<A,…šT@ˆ€UÐÁú?üšÊ¡yaì?µ³›ÎR2þ?ˆÇ#ël @1'o°'@Oìú"±'?ìÕsd{ª›?Ä;å'Ûg¿Ýá\†Ô¿Üi.âìsÜ¿âžaÔU¿çž|øy#AGNbll3FGL J0217.0-6635RBS 0300?ï¹Þ`€u?tHɋäìù?kÓ)I(4ù?fÔ©yÅ?u'\«+«S?kVbï?ïQM¾#Mh?•YÃÐVÞ?Ql=ÏLV‡?`ÙÁ̞Ü?"¿"^¡t?"<àþw7?îµß	–‰?'ujCaHe?°óœõª?‹S'H%å?šk¤PR¥›?ƒ	éiYí?î¾ú(¾Þ?†I6oëê?uã÷'ã¹?d_#äàü?¡Sޏw±±?"¡,šÈ€4FGL J0216.8+0510¿²×¼o"}úÀIÕg–ØõÀ:¶ÿݛQ*À<"YÙU@ñiî†0@­õcÄËw?ÂN´XŒ´?W.0ͤÏ]?•ü‹^öä@…>œÈÎ?ïóg ù	l¿æ¦I«D¼È¿èZ9œÙ¿ú¿¸
¤ô–•X¿Ýв_Ž0¿ïþÖ4T›cAGNbcu3FGL J0216.4+0507NVSS J021655+051018?ïÕníÑî%?pÀn{ç?>ÌØ"€|X?5ZΫa˜W?s[»"àåÐ?o¨†1šß?ï£óÀÚËÍ?…o–Ì"!Ñ?3Ú«XÆÆH?EBövíµÖ?†d:n†Ö(?"ð¡ÁÓq?îêý¼WL?/¼·ˆ?t¹'P•º?]éÅ÷Î?¬êÚ'Ù&?ŽÍ×j¬?ïOØø©?æª÷G9Ì?`gíUܬN?RKì۞~?šRxZ%Up?~²è¿qû4FGL J0217.0-0821¿Ñ‹v,úVjÀO2q`•l
À: ZUÖÀ<t¿û-2h@¨0lYoˆ@+œ›¬™Q?¼ð¢…?À•ÙE¬¯@Lz-È?þ66ò?ïÜ3<mn˜¿ãb€u¿å0éý_;пåv•ˆ'á¿çŽc_öµ©¿ïð"¡!1AGNfsrq3FGL J0217.1-0833PKS 0214-085?ì¦"Íit?®CGGF
?'Mµë9jA?|õD(GF?¸…Äœ-‡?­²ÐÄ?í4QاSà?³¨Ê;¾B]?—,í~b&?žv^˜ó~T?°'5Û,×d?­£Ç>:!÷?ëìh…_ïÒ?¡ÝÀï?œ;¢é$(¡?‹Þ+"p!»?¹Ó·w@?œTq¶?êÙ¹ðñvá? ÍQÀÛTö?­L=ý¿©J?")ÓО!!?ºŒy"tT?™Xìûzu4FGL J0217.2+0837?â>^ˆfÊÀHQëcÉÀ8­43ä3À;é=~æì@¾»Ú(Ö@ì·M߆ä?¤	±ãÃ?¥]™@áÐ?ÿ¶¢Ù´;Ü@ÈBS6³Æ¿Ò¼ççÛF¿ãeøí½]¿ã»'Ê°h¿âë¹VÎBï¿å҉øÌ¿éJñáeAGNbll3FGL J0217.2+0837ZS 0214+083?ï"Qòğ;?"ÆÜÔ_¼B?Gƒa÷]B?G'f;er?‰³M4ø»H?"MЈô¤µ?ïšX\~ë?ÞŠ±òM)?Ew…".Ш?_Ü7l–"?ˆp"]Xh?C,·*ŒH?ï'Áð‹¢@?'âãXÇÍ?msèÑó>"?dñtFZË-?—YDÔMP?'(ÑRîU?ïÂ
¨ãF?gÀ*Z0$?Y!È3H•?J÷°òuç?x­ˆ‹ÁŠ£?d11:Ž"q4FGL J0217.4+7352¿ïÙ֚àì@(âCV–æÀ9͌æ,ðÀ;¨Ó5œ™ÿ@—Èe^ÿ@tŸM¡?²ÒRȤÉù?ºÒ	!¼¾7@Ý¥b$¸@
»ž8¥8¿uv×çvà÷¿æïÖòÀ|\¿ëhª¾¯þ‹¿ëÕjËOõ¿ïûâ~å¹-¿íÏîõì€ÇAGNfsrq3FGL J0217.5+7349S5 0212+73?ïìé\R?aƒa¢uÏ?Wœtã[F.?^ۚì­Êî?M"¼È£?LƒS`²w?îVb',gT?°üNœ¶9?†"Ýz1÷?š+
·ƒƒ?¤ôæHZþ&?«f!"‡R?îÖ"±?•UÕ3‡?ŒìèÍÅpz?†(ß5×£?§‡c¤8Ã?±€"Ü­â?íÃë2l³À?–9ž|ÎáA?ž½XèÍm?+£ÅJ ¬?¤Àn,À]1?Œ<¹ŒBÚ§4FGL J0217.8+0144?×=k†òßÀK5 @|ÇÒÀ8DôètÉÀ;¬šˆ¬âL@ÍVnjñë@FÙ='©?X,€«Oé?°X(àôÌñ@Èí_‹Î@ƒxOÇéc¿½ñ¾xÌ¿áU74I³¨¿ã¤ô xÆe¿âŽWF7ò¶¿æ~c³-¿V¿ìì¿0|uAGNfsrq3FGL J0217.8+0143PKS 0215+015?ï³T•'?uÏ¢âã)?ES"ŸÝë2?=°™jgì©?Õ¡À—d?unñ™?ïÃõÌjÕÌ?€Ñ¡;>'?5²]J¸?R>'èæáp?|©óõôì?€Qä0±dÎ?ïS"2·¨R?'ut&$úW?p`:ÿÌ4?mòOÁ-JÎ?'ƒ«(KÙ?~'+­+÷Õ?ïñ§dŽ§$?JØé"G•&?"梊jÇ?ƞԸI?Zpz`i²?IÏ%ï¤"4FGL J0218.9-2305?ÝàÏ"ÌûÀQt_®¼@ŽÀ:"WÀ±5˜À<žù˜òc@"ÆóÄÞA@˜Ã`<€º?Àb–P9?¦À#Ç‹Ö?å'"^#̹@š?Ĝý¿ÕfÓP0š¿è,ÀÞ'¿è2µ>»§‹¿àÀ;Ÿ=r|¿ïÿþªJl?äcãÏßAGNbcuPMN J0218-2307?ïõØ÷/?U>
úø>?6Ðêgt—ã?8ç%VK5z?Pwð|b?Quþ
ç<?ïÐ÷P'L7?€Ó¿'‹™?+¼p`"ëM?Hë:OÊÎ?v¦tiU=z?€õÖáž/?ïV¸ã›/?x£#]?f"!¡~æ?VMh±Ö†?'jˆßXj<?vdo	K@?ïõ©åÎA?CƒóV#Í?"0‰Ç†Þù?rv´Xæ?Rf$¯rŸà?B(Þr²F4FGL J0218.9+3643¿ì7ƒžtc™À6ê1…ýÀ9œze ì	À;˜	ÿ÷@¥³/³ø@ʅ4-?¹¶ˆèœa?ǤC@Çpl@
f|¼A%@``?°Å¿Àß]ނÐ¿änôËG<¿å=ù*"é9¿çÑ`°D
¿í>"z~K¿ðAGNbcu3FGL J0218.9+3642MG3 J021846+3641?ïÂø"¢Â%?v,J%Û?h w'ÉvQ?e€Ψ*
?rs²åº2ö?n- ž¸U(?ï-=|q×?Âã§h?FãAvWvl?\ìÁža2?Š†|‰~?¤wçÑq?í?x|¿Þ6?žö²%ƒ?˜7ò@Ï£¹?‹?ýƒáe?¯ìšJŸ?˜¤\IÉ­?íËÔ»]˜œ?"ΆÅHòU?pêýHÆÕ}?a†5䞹U?°'ªP†ÍÈ?"BRÝú¥4FGL J0219.0+2443¿êœ°ÞÀÑRÀ@ÿÊ}g3ìÀ:T6KìhÀ<]°<sMÕ@ {ÂqÔ¯?þBÙÏÏ?¹jàHª"½?œ}¿ZÑæ?åT*Ã@LÌQ#ß¿ïW‡Üóö?ïÿ˜0ã͚¿äQ™_â隿àcRµ¯z¿ÜJ±ŸIÜÿÁÈpMLAGNbll3FGL J0219.0+244087GB 021610.9+243205?ï¾°ù;óî?u¨{ï}Ã??CŸÇˆéO?<–ç­…D?~3ŠpèßÝ?tÌýrT‡?‡†­‰?Š˜í‡q½º?A+…@ù5=?TslêâpÊ?ŽAeÊE	þ?‰hDmÿ:À?íá
U3¦ˆ?óý®+=³?w]³Qy?eúuf†6?¯¤B£o?™÷@öÕ6?îŽqò+™?‰KšÛñ·?pÆf­ž¼V?`
 õ±Âã?¥›^ã?ˆ¼¬<PÙ4FGL J0219.1-1724¿ïft€Û\³ÀPã9–ú'èÀ:Œ/•ïÀîÀ<€šl'p‡@74:DI†@ÖßZn
 ?ÀZâ9E›ì¿m;8€Éç?±cDë@ëÔZŠ»¿åPVY¨é¿æ%»`"¾Ž¿ç)%]‡š"¿Øë/þË¿Ôx=({¿ïÿÜßi‡ƒAGNbll2FGL J0219.1-17251RXS J021905.8-172503?ïÛ´ka#?m½FÑ­?7ϊâ¡?1ïOöÌ?p¬ØbuÑ?lc@2û˜æ?ïÇhïÙ('?	i¯S?"¼N7º?6yÉxž?{µ¥¢»
r?€Ú¯­|¸?îžN±¨?~"®Ä·?h¬Zs‰ïE?W`t¾-$Ì?¤Y]¬à?Œe¤|Òí,?ïsw¯²?yS _/Ñ??'RÄ/à?4"k2²‡ò?'æ¾­™?y5üvVº?4FGL J0219.5+0724?è«Óœ¹xÀH³é ÀièÀ:ôBŒüÀ<cÀ›f"@ YC=A@mY9?È/Á#K^£?'ûôW«7§?ÎõŒI$M@¶ÜuŒI?ï©iñ5aâ¿åÒ%fÁÕù¿è¼Çf[~¬¿Û¸‰ÿr¼`¿ä ~æ¿Ûš©CÛ¡ýAGNbllGB6 J0219+0727?ï‹¿§ô‹?'/ßtÓ2X?O"Õg0¨?E!
"m˜«?›òab5?'í1'éZ<?ïybù¸¾E?Š£½Rý?AÅM,7DM?T*÷?Ev_†}>?‰h"\t'Ï?î3š}z?'m5.˜ÖL?m,|«6-Y?Yê#ÕTÉ?ªó–¤TŔ?'†yÇÊ?îû}çÈ¡?€O ¢2¹`?U9`×K‡?D1Ñë-ÎW?Ÿ:ºB9w8?€(SúhÖ4FGL J0220.2+3246?æ¸i OÐÀ:z|¨"2À:‰m–cÀ<QjúIݚ@òÞÜĽ@^ڀêv?Îj'ÅêÛV?Ô:è‰A@s¹»x³@øE×î¿¿à¶l¾o;ø¿ãt°¨©Ø¿ëMª½Ù>ö¿éx՟eæ¿ïÿå(
eC¿ïÿþÐñAGNfsrqCRATES J022048+324116?ï䌼ÝJ?e2‹ÏíHý?L%G™eF?F¶juͲ`?dåñ<[À?b_‹œ'n?îÃ:âÕþ'? …ûR5c?p{~tî ?|=•¹5?¡ÉâbÑÎ?œSýØ/ëƒ?íK™–¬?™dà_ù?–Í¥¨–†?‡˜«Ôš™?¯è'J5?"Wë8"?î¿3¨RD‡?…ÐÃùèLÄ?éÝöd?i¹ß¾/Ë? ‰Úœóü?ƒ'p>e.¢4FGL J0220.8-0841?ïà&˜°LÀNúˆ&ªŽ´À;SôÁœ¬À<´ÚìJ@–@!–L\yþ?÷Π/µÐ?Ôê&yçL«?Óú†c±Ö&?ÿ'~þà¹@W#	ðCÊ¿äúTû½¿ïÿ"Þï?ïá³äžzª?ÒÈÌøk·¿Þ~½_ÇeÛ¿ç:d_¦ßAGNbllRX J0220.8-0842?ïÀ«‰èæa?}Bjר\j?CuÓåa"?>8ÉÀïQ?}ILQ#??|Nªl ó)?魯ëÉ Å?‹Û
<Ç_W?Agrm€ça?TE/í«Ê?…»
æ¿Às?Š'	vn¦?ìÝ	mE5?¡\ˆhßk´?€âg0%µa?rNƒE
`-?¶ûg¯ÑA? x´*M©?îòi¿?ÐÜ`^yþ?AxYv?@=v֛VŠ? "./ò*?½Û^qúM4FGL J0221.1+3556¿ÔôÙ/º5À7|K	éÎÀ70–›¸XÀ;)ûbó@Žn F±ë@Çâ'@¸?ŽÁsR]?¨¿3\"ë'@(}@@ Qg`Œ\Å¿Ì/
3Å)j¿àå!×¿ågûý<a¿âý§*{ԍ¿èKABG£¿ãE5þAGNFSRQ3FGL J0221.1+3556B2 0218+357?®ì‹b?€&ø­ÜÎâ?D"ªÈۍž?@?%Î/_?ˆ‰˜Onà?Ë(î	=•?ïÁŽ²iµ?"qÉ
$áU?A•‰ÐqŒJ?[9[¡éÂÒ?}õ¹<óß?ƒz+ç€Ï?ï%]ú»S?¡¹x¬"ß?}ɓ¯ ê¬?þÈA‡ó?"áøTà[8?†u5K¶?ïøX^ÄOG?Bn'IØÆ?µ8nÆa? Ÿpº?L³1m+öÍ?B€0b4FGL J0221.2-1312¿¨%¦ù@­¡ÀP4 {5À:ý‰»Ö"À<›óÜ܉@ÿB%¿WC@òa|ÚQ?Æ SG$צ?°¬°L¹l?ä܅§tM°@l6k!=?ã¬X]ºn¿æš·¦ÊÛ¿çuK;gµ¿êUü¡PÈ¿Èò]dŠ¿ïø^졬AGNbcuTXS 0218-132?ï}×Ç?Ä=?‰Œ-)z?a`x]
qù?^DRføm?Œ1ðÌT_?ˆAÒV;×­?ïqÍ·à¬?"Dìé¼%?TKH Å#?j"›ŽZ?~TgÞ?'jœG
§¦?íÚàÜI!?'J…ô÷Û?€ÙX5b€Ð?pgmÊïòˆ?®(ëäâÍ·?+ynµI?ït¹Vv-?xŸ~C&?Q%<YÖçö?HJ{úP@?Vkœñ8?wɚƨÀ4FGL J0221.5+2513¿ï0^¶³t¦À@¨û¼¾bÀ;>1ø .À<Ò2º¥@œ9í±?ûåɾ$"]?Е™"Ë×.?Ú3~݀¤*@
Ô'ܾ²@	G¹¢£ƒ}¿ïÿÿ" 5•?ð?ňP†€7H¿Ù¦¿<@x¿ä"éõҀ¿ïÿô!O…úAGNfsrq3FGL J0221.2+25182MASS J02212698+2514338?ïÁÒÃ1®?‰}À{6²?Zf8b9Dª?a5¯À€?x}Nš§a?ˆ;éݪ¿?ïH£ì$f?ŸÚWŽ«?bÚ	ïh~Ñ?t'ÄÅEmò?›{ªDŽch?œ_oÉÁ½?ì9Írž"d?£¾×q8x¹? mØ`*•?"¹È92P?¶*]~Ûǘ? ØÇׯ)š?îÓ¤c4?†Kə§«?rÐ_·¾ïn?bœä
Þq6? k«¡îã?"s®½è4FGL J0221.8+3730¿ç<çFB&
À5÷Yš¦	À:àÐd1À<m?!Î@iohی@êS%A)?ÒÇþÜ¿^$?Ø*Œ»º«¸?úÔLJémí@Édm<ïJ¿îLAœ''?êÿý¥\Æ¿åº<;ðq¿ãU]Œþ¿ïøª*s?qInAGNbcuGB6 J0222+3731?îú0Ċ²?–Ôr#p¹?Hx›tO¼?†"Ó1¶¥7?˜çÉGÏ5Å?'¹Ò†>†?îB€Q+¿?©Î
³N/?ìx#k?'AÑAKc¶?§\óÐ$|¥?¤2Cöåú•?ì%´¡? Ü§?áYC?£áá(€h·?Ž8ÁÛmfê?µýç&Âé?™[(|sG?í¾/µýÎ?–Fâø?'?‰÷|͔èþ?x+üÝè¾?­Ÿ%|JèÒ?"·QîŽá"4FGL J0222.0-1616¿ÉYçû¯ìËÀP—æî·`À:'õˆ­¹À<8Uêî @éÐ[L¬×@GڎVo?¶é9"÷ƒ¿sâX'Ö'?×Vj…YñŽ@
mc-ת?íëw²¿¿åY àŠÄÀ¿çWeÂ|'Ì¿â€3aV\-¿åû]8À:î¿É_A"ÛAGNfsrq3FGL J0222.1-1616PKS 0219-164?ïÔtäªÜ¹?jfÒ	À™?Ds¢ˆ@?5\ûèd?s7*V@š¥?i£S	=»?ï֑͆L?{µ*Qzc?'–K~O}?@Ê@Í~i?xâ[LâG?zùtV@#·?ï#‰kÚµØ?~Í"ݜJž?fÈ*T®?P‹_ͯ²Ÿ?˜µÍBŽ?}DiÁW»n?'ˆø?kјӗlÃ?IšJÖîîk?8§Ÿá7‰*?†Ã'pS
€?k9ð®™Y4FGL J0222.6+4302¿Õ¨Ò?05À0Ãúñ€À6¢7Q¥åÀ:°"±"L[@Y³Ã¼Wà?þPKŽz??¸ì^ý*?¦d'‹‹@Og+ˆD@B{Ÿ]©¿ºÆ}A8m¿ØPÜfrÑ¿àtÐ!#~¿ÜÈh¤".M¿â4áô|>?¿ßuAË|jµAGNBLL3FGL J0222.6+43013C 66A?ï;µ¦°ýÈ?Ìþ[Wí?Cɯ;¥ì^?>¸~0×ë?—êý°v?pgŒíŒ?ï¸Óù•?‡Û·Ñ?H©#i#œ¹?g˜F>±?€@§‹'`ú?†ÍÍùØ?ì¼mÍ>§?¥j²ŠÑ!0?†ìñþxô^?cœ€¸ß3?·>óV@Ä;?¤{÷¯Enì?ïÔ½T>žÅ?h]´Ü}?#²ÞèÔ? R&۞ïÁ?u¾ì±X?h*
î
?4FGL J0223.0-3447?×ÿÝá:ÀQ>þqŠ†×À:ù]Ø"keÀ<²Ÿô&­ê@`À"…b@4:<;ðq?Ñ+ºûéñ?Å¥o±"‹?ñÿPÈooú@	û2:å¯?ïË^£#†¿Ó0¿P‡Î¿çšß¿Ø¿çkº=©î¿ïøô=Te¿ï;f›ÖAGNfsrqPKS 0220-349?ïQWÑûU
?\"86KÒ?f:ü¹õ?c¥¥´+­?"r5Çj?ŽÂƾä '?îôè4>®•? Uû†?u?jßQ"úkÛ?s²@ÚÈR?žSÊà#?(֊ö–?í#÷çú"6?˜¤u"±?"ͅM©§?ƒî"s
"æ?±ÜM^×óç?"™'"(W?î6˜.Y?bøi@V?š}(Ú?~2¢Â±~?¥:Ÿøû%¸?ˆ#cßñS±4FGL J0223.0+6821?èm
îïÑ#@ïÏ_ND1À9ë¼&Œ[ÃÀ<Ê<ϔ'@ —W´?þÉÎeS@ð?¾¨*+!ÁÇ?¹Fho*/S?ûàÇ¯;@E®CÊ°¿á€À_+3µ?¬–ÄŸÊ®¿ã.Ò{bw¿Ô.iàCw#¿âúã±à¿á6YSXmAGNbll3FGL J0223.3+6820NVSS J022304+682154?êB«äëM?´Ó³+"n?ƒnÙ`'—±?{I]‹ÌÒ?žbٛ)Q?³Æ0¶W½?åòŽ!Ș?Æác/ë`?zE+Ú>?"t†•bü?Ó²š§¿fÍ?Ɯ ç;'?éX¬½¿?¦T2Le±?""¶ÔkA?{pc˜¼?Ç['¿¨¹?¤Èá3Æ®?ë øÁ©4i?˜¾ãö  ø?'§#qæ‰?…&¡A»ø?¿®P)Ùã?—ß99öá4FGL J0223.1-1117?Ú ¤).f_ÀO¡Ò|96'À:6–•[À<}Hé}Ý{@ f&áÁ&?û*|«LI…?Ëkûf=K»?ª×Äøm?üàÝ%	¤Ä@\PÈðIT?îI=@}H«¿Þ•ØCùT¿åµmÕÆp'¿ ûsÿ+CÑ¿ás~§Ð¿¿æb»K›	AGNbll3FGL J0222.9-11171RXS J022314.6-111741?ï"5Zàög?~ƒî:‹j?Btë™Ä'?8ýû†
(?ŠZ–ÊV?}ØFfi8ƒ?ï¶_5À!?"z}ì[&?0ž4‡yRà?IÈHqbŸº?ãJNT-z?ƒ¹U6‹Å«?îw-m¦<¡?ñÞà6M?fjåwŒ!Ï?^h÷E§Á]?§&zÎ#sØ?Œ¸Þ2ÜN~?îÿë
b¬
?t£±"½?W>&Ro…d?Mªý"keŽ?žŽ»îƒ†-?T`·C‹4FGL J0223.2-1653¿î \ë#¶$ÀPœ!ÿ.HéÀ:¡'&цÀ<,:ñm–@aĪêNé@(Fya?ÑéQò;?Ûbs'žÔ@	¬s@i|›@	("ÌUX¢?ëÚ7ïZ–O¿Ù1¥^ɹó¿ê"÷€Õ}u¿í+LŸjéÙ¿ïý—ÛSxM¿Ãˆ´oõ˜AGNfsrqPKS 0221-171?ïÑ6¹Ôü?vŠÝËÎ?nf–s/³7?r!äXr?`b¯·Ô;
?`Ô½›PA?뫉Ì=?ÄV܆6»Û?­Ç·=cb?ºçñÜmí?³Ã‹ ì]?´¶'ûÝL?ë5W}Ñ©ë?¥¿$‹cÀŒ?¨ñi}¨Tb?•Z¯ïÂý4?¹ÜRž†{? ̃ž?äØ;{¦:?²sOkN?²œNÝï§:? a×r¬?Ѩ·ÑŒÉ½?³|æ6¯C4FGL J0223.5+5415¿ÛD`™À'oÀêÁ5¿ÕÀ;UZ'ÇÆÀ< ×Ê,ß@!níËuì?ú½ý¬h©7?Øy*"é9?âD Á@§@=\œ¹Ë@}µ…]w¿ïä…CÛ¿ïÿêњ'ç?ð?Æ´ž˜1Á¿â¼œW~¿æ¤À>IëAGNbcuGB6 J0223+5413?ë ­á܆D?Æ"Nk)ýš?zh?íc}?‹V«
éÿ?¬]6Ž{Ö?ÅLjUÅØå?á	ü½âñE?ËðԈÀåz?pÁÃÁõ	?"d¼çvžé?Ý©
+¤?˨ùh1Ðë?éüZ?­Fä·Çµ‹?"‡¥ç®?ƒ?q¢rý*?ÉK
õm?¬T§ŒÐÓÊ?ìõ+ù\ ?¤ÕÃkYº?oyÛI‡?l0Ýöòï?·]¬hJÒØ?¤¬‰Ü$"s4FGL J0223.5+3912¿íVÔc«1XÀ4BÁ HàDÀ:†câ'§åÀ<yˆ¥U@²Š}òÊ@¾4[Q_n?ÃGÃx4–?¼b	4‡=?ö®…ÙÚ@¶œ€SÍ]¿ÕÜrÝGÅ¿á‡gÓMðN¿år5a¶©J¿àyêaÞv¿ÞD]·ì¿ïíE]'<0AGNbcuB3 0220+390?ï>'¨ã¬<?Žtê
f»½?Sµ©¯å…—?MSx6{×4?–ÿ°HŒ ?Gò¨4?ï>—ÔkƵ?–Ž×"=š?UUq[Ø?gL1ÔÒbU?–Ü…m0¶?•àÎÉKQ?î·<`Þn?8b9R£?v§%wÂq?c#e³È‰+?«§Šù֖?¤lgëTŽ?íÞ¾®	,£?ªhž20…?wŠ,)?e~5óÕ?¯"ќ£Õ?ʂjMµ4FGL J0223.5-0928¿ån>LjWÀNÿ‰?¯BxÀ:ã‹+AÍ*À<¥­ç.wã@$£ÞlŽ@×:ÿ°Nè?Ì
,"óŸõ?Í4M¦‹ð@ð÷"0{É@(Ätñ¿ïÿÞ!ˆæÄ?ïÿíáoq'¿ããªÿójÆ¿áTî~ù/V¿é¼êº:#¿ïö…Î
ºnAGNbcuPMN J0223-0925?ï€ÉìHY?'W3žÄÈ?pÊ%|ˆ;?i]pgÖà"?‡h´r/¥³?€	³Hl?ﬤ4?œP\VÓ?k6rûPn?w¼ï,Ivö?™#¹/R?˜tÀ–»·¶?í1‰ÿŸ"?™T±0®nr?•·ø*¿ûo?‡ÃŒÚ1G?±±øW¼ƒ?'å‹?î:êfúÀS?Ekˆ‰ª?ˆ\OçÅ?vfÅa‹`?¦:E–'òÓ?‰†mgø¤4FGL J0224.0-7941¿ëtrúÀBAþûôÅÀ:liÁd¹¾À<|Jù"–-@J&>Ù@%Û[ÛÉ?¹Û©´nÝ¿™1¿ìÞ?àæzÕéV@Læ/ŸTï?í"Þ9Û¿ä©Q†¿å
$¡u;¿å¤=ÔÌË¿Óþ_o×(¿çˈ>¨\UAGNbll3FGL J0224.1-7941PMN J0223-7940?îUþ\,z? ˆj/¾sP?l"	§x?`dJ•Õÿm?¨ÖïJ2Ɯ? 
‡m⯈?ï÷Âz?œŠHJEÞ?HÙ^˜ã?T?ÐÆÛIœ?œ @ô;ÿ$?œ#§\*Û?í¨'ë6,Ï?•ˆæJ'ñ?~sºú¿´?j€H
ª?°Ûqjží?"^¡—÷…?îÙӕó"·?ƒ§>³·˜?gד"°Þ?WêZ^ûE%? åMg'Ë|?ƒrU3…Ì<4FGL J0224.0-1850¿ËUûñ8ÎÀPËʖ'§]À:ÚlVjoàÀ<•?†'Í@ gšÅ=·F?ûµ1öQo?̩͜çD?ÑŖb,šé@)à¤&?úæîÄnYz¿¡%uŸ-F#¿ÚRÅ؈?çHšÙ4º¿ÉH‡r¥¿á•îê.¤¿ïÿªÛ
}2AGNbcu3FGL J0224.1-1846GALEXASC J022404.29-185029.9?擄14¦?•'ùf"·?lñÔª¨M¾?e½'ô‰Œ?š-/d"a‰?"¥Ü=b™?îÈ#"{?§P<Ìé5?uÔ¢ï÷?ˆqô%Hê? Ä¹iØO†?£™Ð"'Ð?í!öHóüd?˜gǵ걜?NšëâÏï?'*ô™'?²Ü¦ýghå?"ï·å00H?ê´«l›¾?¦ŒÛ
Mü?À/ªo?†û¾Y½ü?Ã1P‹¦ K?¦sªéÜâ©4FGL J0224.2+0700¿ê~|¨.ÀH'$cŒ—SÀ:wpoÔ¤2À<F'ŸªTÓ@Rý8$‰¢@êN7›wÀ?Âc\›·V?±áÁ'ýö?îí{ì	©@«ºCf§?À®|ª }¿âÁŠÿ¢âî¿æ'~Ý«—¿ëÙ—Œy ¿Ê
#D}³_¿ïþËí©¼'AGNfsrqPKS 0221+067?ïFþϱð®?•ŸŸ¢·VK?_!~@]b?^_R€úw?•.'íäT?"ø8ŠoKk?ï?R¤çg?œ2ã
¬_?S.ZkÃç?h©Ð"'J?–âżVÝý?š?TŽØç?î¨M¤FT±?ŒžBO(Û?mõÌýÂÃ?^Ó° _:?£›È뾓s?‹5etÖ¾?ïBBþ/
?| M¥;NÃ?Kq›?œÜ¼?B•-?–àêÆ=7æ?{ó`œ!
%4FGL J0224.2+1616¿ä±Y÷ ÀDü;OagÀ:y–JYÀfÀ<J¶4‹@²($·Dz@jlBHyì?Á=z^ëÈ»?©ËndÁ˜?ê´¯ÕEAS@xƒÚ?ï;2G¿ÍEäßq¿æóÇb¦ÿ¿á"Þt"ý¿ÞÆlÊS¿àÅFÞ	5AGNbcu3FGL J0224.4+1615NVSS J022411+161500?îVÀï!±Ô?œGq­wŒ—?m¢…ûz3?au"7ÊÂ?¨¹È®-?v?›gÌ%e?îÝob©Ýô?—^|Þ¿7«?\0b" ˆ?aá]]€´Ô?¡GˆÚM³?–v"zUš?íVl«Ú?•—ÊÿéQ,?'6̶,qÑ?pÊë=Á?³őø?"/…8L?ìôî†)R?çï?–%S?€á‹(Î$?lXw9^È?¶<Zižà?""b;4FGL J0224.9+1843?áǾ":ŸÀCn¾H¥‹À:ìxc¾ìÀ<	haQT@wv./"@CEÏíé?Ç`ü" c7?Õ½½eP½@i¬ÿ§ël@¤yÊl˜¿Óp¦{RF¿çF—ɵÁ¿ì¯D]f¿ïÿÿ&¦³?ïÌ"'áÇ0?ìMÃ\á'AGNfsrqTXS 0222+185?ïÃÔÌCÉê?¦nE·¥k?Ztɛfő?ƒ0N©.÷?wxgwAZ?¡ÁYªÖ©i?ï:ÞzOÛ?®©I±Ô;f?sãGHÜ(µ?•ÎËXÏÈ?˜?Ò^~úi?¥íÔ²¥¬?ê'ó©ùÏ_?¤è 7O?¥t{ý¤ï?"£'-?Àn9Y@?¡pøΰÎ??ïíý`•RÏ?c/¸¥²ú>ý9ír9Ãý?
š€Ó<1ç?aÈ+È½ã?bø½AèL®4FGL J0225.1-2604¿Éùj´¸óÀQCÙ+à‹À9xöžWn|À<oKG&/?@f,êįr@ÚÖzËx9?¬¯àš?°ˆ©¡x—?üâqÊG·O@,æyq0¿ÒvÊÍL'¿ã™_÷·\¿æúK '\9¿æ˜§8Ϫ¿ì÷Î8׋¿ïþÊ@*'{AGNbcu3FGL J0225.2-2602PMN J0225-2603?ïëcS䜻?Y—¶–â]£?9ÈÛä/à+?-Àþ»Ü·?acžÝI_?XG‹¥¡§¨?ïÙp¶¦¥?}Ì,â{?%➬ý?P¡"
ßL¿?r˜Hl?zÜÔÑÀBê?ïR%âç%X?x›Üì^B?i¼r_S€?VNúG÷V-?'ƒµW:ŠÒ?vµAWŽ3Ó?ïõȓ4?C
4'ŽÊé?2²lB¨–¸?(7õ¬ÌW?O"}ÁÛNÛ?@'Ša[AK4FGL J0225.6-4502?ÚÐ%æÞ4ÃÀPNe¾ ºÀ:ËY%5C¯À<niØá®@Ú}¬Þ@ÓÁÛØ‹?ÁÛ«¢Z³U¿`7hÆÕ]?'Ã`Áû@á9|Î\Å?ëÅ3 ïò¿Úˆ€Âˆ%¿èri>‡û¿â?–ƒd£ï¿ë}·PcÅ¢¿å۞¡Á0aAGNbcuPMN J0225-4503?ïÞ;[9?i¸Ò^°.B?CIÑÜ÷á?8÷·ß|OO?lò0á	U?h?RĬ'?ï͒bX"?€Ïf$œ:?*d«ú"×?Có€Õ›Y?xc® ô×?€8<cðï?îöå1Æ}?†¤fðx¡?u2€U%S?qjx}è?›Ö½Ä}Ûn?'Èx'°Â?ï½ÊƒÉÄ?båÜõŸ8Ÿ?EÊúÚ>?4ƒ®‡Ë‰?~xU¤»Â?bn¼@cB4FGL J0225.8+1310?•÷ƒu9ÒÀEÑ¢Æi}À:NÈ.›À<Rû15,@ü'Ñ*T'@üÛ`
†Ñ?Ã7²žÎ6Ú?¿0°Ìæøó?úÆ&Nyá@Ú_‡z¿³ùû€Q¿æ(¾e*ý¿ß=ïN×Ôh¿Þ°JJ¦í?¿âqâE"ï¿ïÿm²æAGNbcuNVSS J022551+131046?ï—Î'Ê?€`=춮?Vq¶ÖÞtR?OxiM5µO?‡>B1¯s?!«RÄÔ?ïZIR'æK?ij3Gíÿ?@
Zu˜)Ø?LœÀÊ=XŸ?"6jÙöuU?)Fªþ.?îÜðÂï?‰íµj¸¥l?n+¤Ilñ?c¾ý÷òEO? N9Œ}Ǒ?‡§º¤>›€?îËßñÞ?~ª{)ø9u?e§by$ëÁ?O±ŒÓ´¼<?¡çŠÆ̳r?}«r‰ŽŠ4FGL J0226.3-1845¿â{ìo ìÀPª¼£nÀ:¨"7blÝÀ<l¥Ö¾¾@ p®øU@¡Ðº˜ã?ËÇrÅÅFœ?ÉAóU?ù¿g¤T¿@¬äúëï?ïÊBy!T¿àâՂ}ô"¿é\sÔ
2î¿è=•ø$il¿ïþÁ¦þÜê?ïñ"aÎüþAGNbcuPKS 0224-189?ïáùë»3`?fÏ8ã8Ù?FôaÞ§¸w?F
,9W§~?hHûÍ"²k?cëùm绛?ïi'v¤øi?—š%*Ó†?Z%:'´Õd?rŸ9RŒÙ?'-]ˆå¥¬?"¼´ƒ€?îÂYk #o?‡OԂwÌ?{
·fÒÁ?qVâ4éJ? x²a=nº?'悵©
-?ï=
˜'?qêLg•;?IìºNõòø?=ëÅÕÅ6?‡ñµ_?qVW`}"p4FGL J0226.5+0938?×kZLãĜÀGMÔ{í·(À:lôI:ÜÀ<a&õ7O"@<«S«MÌ@Yúb1M€?Æ06(°ù?¾ÑGA_Y?úß;ÒDÜ@"˜ÒtV"¿çØ÷°Õu?èά5}O¿ç›©¿+¤t¿Ê,Æ`¢¿ètõ_èóÊ¿ä{aT¯AGNfsrq3FGL J0226.3+0941NVSS J022634+093843?ïãÎKâS~?m	t±h…c?3GÆyl°?8DÇ쮒?iÎË$ÝSË?koC?€r?ïÑôŸ™"Ë?}9~™¯K?)V!F¢rt?D²·ÓšÚ?v:ÿ)9†p?{éç°;2?î܏Ÿ>?‹_^ÝâÁ?l°9s‰t?a×h"å?¢tsnӊ?‰"Kþîò»?ïäïw[­m?R¿EÞÜ"?1#‰aüì?#jápHú?hï"3&S®?Q.#²·3Ý4FGL J0226.5-4441¿Ûã2¼ìÀP6Þ¹^[À:_Í¥òmÀ<uW¿Úv@ Xûâäç ?ü̏	óžÉ?Áçt†B$?Á0ŸD©RI?ý0 Y;Û@5qß@lØ?Ó_JrÉK¿êС£SV¿¿Ãz
?åH¿ßœ{¡6¿à7#"ú¿äÚséܨAGNbll3FGL J0226.5-4442RBS 0318?ïÓè"ß±?k[6Š"ª?>nªnÎÉ0?6Á'Ø–,?t—!#:s?jÑêæ¸?ïŸÇЊ?‹©8ÑZ]?8$¿«ÃYU?Fÿ¬ãÒ¥Q?‡MΞBØ?Šúz‡?$«?îÔC
?ˆ¶á"!?d•Oʛ?]´·¶ˆÊ?¡vFßb|n?‡–".hè?îÓž¶?ƒÑÏþÄÉ?T)
ø;LË?D+{ê3¦?¢,ͼܳÇ?ƒÈI¬CÁ4FGL J0226.6-0553¿ÓSŽ¿ÃÀMz
í(ŒçÀ:t`§	Ä¥À<—À{†@ÕüT#î@ä;ÜO Ð?»¹J9	6
?'p%_"—?Ôî16ñL@¥$Yт"¿´¡¢¿å0¤ãy·|¿Þ'Ðý‰H¿åÜv"œ;¿âÇîvjÀh¿ä§­­"AGNbcuPMN J0226-0552?ï ·ÛôJ?š)hIäʋ?^o/õ2Ú?TÊôŽ"¥?š	/£‹?™Ñ˜îSwÿ?ï¿°ò?€—ÏY˞ã?.݆:¨€B?Hô§è?'MRBÖ?îâü?þ
?îÜN½KóÌ?‡6"\hì?tß¾QI?pv'Ìg©è?Ÿ>h&í@\?ƒˆai«°?ï Y1"ˆ_?l%P¥	t?K
NzZ!?;RTô¨È?†9³<R½?k$^\ˆùM4FGL J0226.7+2312?à:Qïz»wÀAS¹bŒ½À:´ƒ*ÂKÀ<aÝ6§[ú@ 6՝@YbÝDê?Â˅úÖJz?—‹|ËW¬º?ÖÏ;üZ"?üà/€ L¿ïRW…øÒå?ïÚî}÷|¤¿ãϱƒ›*"¿äŒé‡îvk¿æãÕAæT]?À‹#õ}›AGNbcuGB6 J0226+2311?ï.Ÿù?Û¤|6n?VCÈsou¼?L'9àÆFÅ?˜Çà¨%…?€z€´?îöéþMyÀ?™j[ZØ2?_'8å›St?mÄ0–¹±£?Ÿ)¬§÷¹?—E—ã×Yº?í·/Eš~d?"({ɋÆ?	¡uÓÝD?o.±å—ƒ?°Uë»ÎÏ?'X‡@YÉj?ì¼Ñ}`""?™oÔñÎí?›zŒ&5?€Ó›ð«.?µò•qòU?˜ÒšçpÁp4FGL J0227.2+3928¿á!‹gôËÀ3Áޜ)¦À:Qnf)À<
ÏCŸ'@Ê·Í·-~@ÿëJ?ÄúPþöÅ?£"$à_%Õ?ØzšÛ@
ÈcCqCå¿à«RÿU¿ær»ß>¿X¿ê_«+'U¿âÄC@Çpl¿ïɧ~^ª°¿ïâÁ*ØßAGNfsrq1FGL J0226.0+3922B2 0224+39?ïð)+˜ýà?\V5•S"`?CHôü_ž?A&dW÷Z·?V	.O¼¨?X±¤ºj†?ï¥F¤að?Œ¤45ht?<wÉÆ$?WÙv?¤T©?…ʽH¶co?‹^½i{Í?_fl?ÉƒG¯aÁ?yAŠþÛöá?r©®SqC/?¡Oœª.j?ŒÄ	^ÛÍ?ïMC?Œ@?z[y¼jd?bë~"5í­?QË
|œ¢?"ú(J§ºG?xüij™4FGL J0227.3+0201¿É!hì§wÀJgãŸw),À9­ÑI3O¹À<,Y4©@îÞA>c¾?þÈ;4¦?²D
Ëð"??œÃD¹?ì¤ò'Ð(¢@4>=¨W"¿á¢žA-¿àÂñLO¿àŸÍàÉ¿ØKêd7b¿á‡Û+4a1¿Þ`ø=hì(AGNbll3FGL J0227.2+0201RX J0227.2+0201?ï¡ÚUß$?'ƒ)n4?be-õ?X(þÛU–?šR9
?'}n¡ÌAÛ?ïƒÎÿ|?'*ü?D߉ƒV?Y‡i	x؈?ñTOøfp?'o–t»|?í$ÅoaEf?œ»æV©¾õ?ƒ¾w¯kM-?tâóÖÄÂù?´bk ?šhµäUE?î‹m&‰Ð?ŒŒºÍç
;?o^Êȕ?[؟àÔZü?¥SLVÖl?‹˜}"/f4FGL J0227.8+2246?눕']q1ÀAvÐâ2À:'3"«CÀ<S¯s²M@ïæÌRT?ÿI-U£ "?Ï0šgó
?Ë›Â߁@kq'úä@kÓ}–á¿è‹ïŒë5n¿Öa/šÍKM¿á‹öþÏ~X¿ßØxýlÒ¼¿æѳ¼ZŽÂ¿ïþû=x†zAGNbcu3FGL J0228.0+2248NVSS J022744+224834?ïåëKæËl?`Ñ&Ц&?=ã"?F­Ì²?fb—·sÓ?](­é'/M?ï°úyåy"?'æ§Ùz?0mPÄ» ?DÙ×[qÕð?ƒA.'Ý?'D¼E4Ï?î!úŒ?Ž—_‡ï ?vMïƛO?kÒyôQÑ°?¤4O§ƒÓ?‹&å&Þ.?ïmè×d|?u<¥;[ò?D^]`÷½?6þìŸ?'Ÿò*vS?u¿áîÇÇ4FGL J0228.0-3026?Å¢1BÃ"ÀQ'N;Í5¨À;óÜ܉À<·‹"- Ê@MϹ'0¿@î#yÌ?Í×¼w¯d?µ±-œ"`?çؘ²é̸@óÔyêQÃ?êDXŠÑ ¿Ûw"}~[¿ã*l»>¿â³_þÃ?¿åª""Žö(¿å0´hQøñAGNfsrqPKS 0225-306?ïÈY'éW?sšø†÷?5ŽX0Qƒ?+Ê´.œ?zžm³‹'?s厽œ?ïÀ¼Î<ä?'fLAv?0"œâ…(?JcXÕά5?~§çÊÁ$Ø?"M'÷Ž?îà¸Qmõ?'GÙö®™?e§ÌãË?Uh zŒ±? ™þ'Ð7"?NAk®–š?ï­OWØp?kÉSÖۏŽ?:""š&Õ?.wÃË?ƒ×ùÔ?kÔ¦'òJ4FGL J0228.1+8208?èÛ¸¶H­@3뚝¥—ÕÀ:¾R}{UâÀ<\±•+v@je›»1ð@" ß8´?Շ#	ðCÊ?¤k·^%¥+?¬ûŠûF1é@¥CWm¥¿ÖYì x±¿è¿¾ëbº¿ã؊:N¿Ý$þývÑ¿ïÿô╋î¿×·0ÃÂ7AGNbcu3FGL J0228.5+8213WN B0220.3+8153?ïÓ,ïàÆó?yÍ}@nov?<G=n¡>7?9¡²€?t¥8²s'?y1¥|'¶E?ïµøš;ó?'˜ÕÂçN'?@ÙÎý?W?S=ÎA?t<šQ/E?ƒ6(à?î0†à±¾í?–4€ Q6r?|옮SKÌ?v;V$!ر?©Yþߧº?"ÀÃ6LW?ï¾V#ü?g°ˆh5ž?<¶i¼åMó?3"#ÇÎy?	‡f#(z?gšü¬Ï/@4FGL J0228.2-3102¿ï«º0ÀQ"gßã*À;C—'h$­À<Ӂ¶NG@tãÞaIÇ?þùúnƇ?Ï2·¸=žœ?Æ@b†2¼?÷š™ÄaÄ@?þ¯áa{¿ïŬý¤†?ëÊGÅwÄ¿Ô
=¥ýÖ¿êQÎ(í_?µÿjXäG¾¿ï÷£:,K¸AGNbcu3FGL J0228.7-3106PMN J0228-3102?ïþ˜
Ë?ˆf¼›5Wd?S6õÅ)ª?TQ¥¢dý?†{[B§Ö?†âiŽˆ"?ïXøuBŸ?˜¼UŒvx'?TôèïŠê?h'Õ{ÿ?"'®¢^ý?–Ü®ÏÝM¸?íÀ/bx&i?'Ìʑ)>?ƒê
êÄ:ú?x€N³ÉÍ£?¯†]̊ ?ƒ~#Ô{b?#ñ~<?'*5fçE^?[미Ñ?Z±j䏙?¦•Cj[²?'òˆ6ñ4FGL J0228.3-5547¿Íp¸
.=fÀL9BÜôb=À8$_Ñ÷®ùÀ;c¤¡4˜Ž@Z4!š¯n@κ'®š³?zùà V?¼âW–>ñ@!±>›A:@€yMHÞ?ë°*Öm_¿ÛœEE"o¿ãZ¡Ëi¿ä!»qZ¶/¿é1ÿ×f.¿ïÿ{uÂ#üAGNfsrq3FGL J0228.3-5545PKS 0226-559?ïˆËP?'
­GVñ¨?qà#ºŸ‹ë?sÖJÔµÿX?"Ý(»j¥ã?{—KßË6:?ïyöv»F?•E\æ"t?J"ä8Ì­?['$tƒ
¨?Ù1òÜ!æ?•|¸ÙÝâ?ìêÐI´HÛ?£\U½EAæ?¦¯I¹D'?š1e¡F=?ª£±«wWÂ?š´ÓŽ@§t?ï[RÂupe?"ÑÊCU(—?`€b§²ß?WŠ¿ï-?''פüý?ƒð:aÀñ4FGL J0228.5-2234?ç¾Ì¿$²ÀPã8`™ËÀ;i+Õpà=À<ÎÀMb‰b@")øL‹@Ægeiç$?ÓsšvL?ɵ˜RÇ£?õàèÄ3¡@+ˆª&À?ïÿ-½R†`¿à÷
}—"¿à8ÝA90M¿äesâ¥Ò¿éµ_B…¶Ž¿ïôó'H¡AGNbcuNVSS J022832-223350?ïL?²A«?'8GôȤË?g·´%þÉñ?bµ÷ô‰Ñ?"†!"÷ñg?0ÄN(×?ïgúß/ÓR?'ùëvƒ?VKr&Ú?gìU_UOD?'›ì÷¥c×?\rÍ7e$?ía%fRÓ?•Ä4§Hm?ð±šl<ï?í"¿Ì«1?°º¨fÎX?'#«Y/P?îø£Oz%?'ÅJUÿ>ˆ?fÄum¾¸ý?Y(ÍÌ_?ž
¨Xäx?'^ü¶Þ4FGL J0228.7+6718?ïoߓùǂ@Ã2Ál"À9´€JœÜÀ;€R'KÖ@WFbåÓ@j_ºzº±?À$Ù~6Þ?Ê-_Ÿ!î½@	ýfe§@zâ¾%À?ÎÈ2É«Û¿Ý7‹òç鉿é˜#wÔLô¿æ$Ç_¥'¿êaš#Ø¿ïÿ˒:)ÇAGNfsrq4C +67.05?â•ÁI‹ˆc?Åz^³ÃB?Àú¿_N?´Ð¯¼âêk?Òƀ
9H7?ÁljXׁ?Õ
?é«>?Æ{J¦põ?»û›•í?½¤Cß°?áûF¬—w£?ÅÙû"sü¡?â@®Dà?²üa_7?µÚa-Ñ£†?šƒ0ÙÍ?Ö´s_?°¨¥¿e?ß®§@f#R?§ž€¥Ü?¾Ô:ɍÂ"? ø*jA?؜J
6l#?§Ê)«tñÊ4FGL J0229.5-3644?܌CMeA+ÀPÊW)²€ñÀ9/»£¯À<TPâp£@gHûF‡Ï@´ž¢íÖ2?ªý¼¿õŠ?ÀuýG¾Ûs@ݺӦâ@[¥…`&±¿×GÝyÃ:}¿ãº{&Á¿èkZâ#Ì
¿ê>šš¿ïÿö?ŒÝÉ?ïþüà:è´AGNfsrq3FGL J0229.3-3643PKS 0227-369?ïð²Éõâ8?UeRKGÅ?KKîš&b?MØ$Ýԉ?Pôuî{¬?G¨•?¹?ïÄÙÅ6J?…¨ÀÈÄÚ?A]ÝçŽZ×?_®å0½ÇZ?{ga¨
@?ƒ$z''Ï?î…Ê)'z¯?–ð™D>4?Ž?Däo?Š2¯é"?ŸÿJ.7ç?'ÊG(Ë+8?ïú$
F*å?8tùjL¦?""R
ãÎ?¤_Çjö?BÎÂd›†B?5ÿÎ̶4FGL J0230.8+4032¿Ôӆ8Ø}tÀ2€V>Ðö'À9^9ßõž}À;õp­è7@Owbâù4@r9`sÞ?²uFþí|?Áÿ_C}X@
ÔF"ú@´Â%~ê—?íY!…Æ~¿áò•S¹»¿æ­GÌGl¿ç$L£2¿êӆŁ~ñ¿áÉO?ÙAGNfsrq3FGL J0230.8+4032B3 0227+403?ïƒÊ¸"äÇ?¥»—Ü!?nû¯ƒ¾Æ?llÁIJó¢?‡NfW3?{ŠNõa?ïÚ蒵‹É?uÚ¡óÜi?+ï£a²ê…?@pØÐæï?q¬9Š,"?uZeP|œ?îΎìGZ[?Š?W¥W?€(Yíê"Í?u´šÁâw^?žõ€j'?"S‰ùyK?ïÓ>n~›"?`ç
HÉK?B6³¶JR¡?3'ƒ]ï?tòIèëñ?^M˜*-§4FGL J0231.2-5754¿êÃøvZ
ŸÀKJGìþ›|À:ˆ׊•ñÀ<›Î ‰ãC@ ÀWH'>?ÿf[~«Ø?¹hgGŒÜr?wôMcS?Á*±"qê(@@œ5UL¿è1}ˆ¿ÔÔBÃI¿áÌoD[y£¿Ú[h¢×0¿áf¢vb¿ÙK¯RiAGNbll3FGL J0230.6-5757PKS 0229-581?ïÇ8xÕKV?zDË`?Ayscµâ:?C=Ø5NH?z4•(㘧?x#ŸÙU  ?ï®";ZŸD?" '2&ï­?,àYíãÉ?>Șæõ?"§ðwž?ƒ¾D©.?îpsDß?ŠB€ø£Dj?qJãŽ??[‰ýîáóÝ?¦ÏoM=š?ˆ—²œâ±ï?ïXÍ÷Mh+?xÛ"t¹áø?Rg
~‰–?Aãýò?"¿Ð>q' ?x'假hº4FGL J0231.2-4745¿çu}ÒáÀNÑ}àÖo
À9¼<ÛR¡ŽÀ<wš‡Ö"·@W´.o˜@(0 ±»Ï?°sHÞ&wŸ¿—ápa«°a?×·ç"
›õ@LJڪ[¿ßnÑ"2w¿åhªC5ö¿êB€®I¿æhÈ@vÕ¿êæ°£¡Z¿ÍÆRIÎÖAGNfsrqPMN J0231-4746?ïê0
Z¹	?g­øã~ƒH?PâL	ý?aØ]À†`b?Z½Îþ"_6?[
søØ?ïØõ2?~'äe2LT?(ݪÏýîM?OÀ{@dÉ?s.˜òwØ?{ߌƒbŸ(?ï%TyÆä7?'"%Š––?h^€CÜÚ?aÕB=ÕM?˜I ¾§ÝÓ?€&	¶†Ù?ïó7˜ $?IxS'QÏì?8&Ë4>7)?2"É5¨Ï×?S‡òÚ,Å?D÷^Ïÿe4FGL J0231.8+1322?ïøL8ÀE^Ž`€sXÀ9@¬ï·³`À;úØPŽÍ@?*^ù4µ@F1!àûX?¯¯4'àçÙ?ªØæ`œ¢ã?öÞ¿ù³?@ʚÒÔ£±?åaUðÍ]¿æ܁u¶e'¿ê±]À¥w¿á¾«¡Ú¿ínTqq\d¿ïù>JsAGNfsrq4C +13.14?ïî¥f†Ð?ˆáð¢è
?FA‰æKBÖ?nw?W"ný̾²?'P5õêK?ïÏýLiÍ?x¹cd·Dô?+ê9"a?AwÙÓÜG?w)Jy´…î?w¼€»¥î?îðMŽñTS?Œ"q^•9P?|±ƒ~c—?}¢k'…?šÊÀõܝ?†záñRå?ïô²°XÄ?EÑ֚Öx?3à‰q$H?+«xu–š?Qèz<ò0?BB¯]C4FGL J0232.5-1118¿ØØ&}ÿEÀN½u6
À;FϐÌk~À<³ãcGP@!#T33@?ø~ÃNžÊ?Ô—d54?ÑøXrÇ?ÿªœ"¤?@Î2eWó‡¿ïÓb³S?ïþ!†ù"¿Ò£*g¿Ç¨·aßC¿àMÛÀ…–­¿ä<×â)«JAGNbcuPMN J0232-1120?ï·ïŒ²?völÁQï?Iœ×¦ú?@盂R˜½?€l,¸?v.FèN"–?ï©<¨WZ8?‡#EË}?5þ-h2¢?Jº£@37?…帾/ä?†XÂíßÝ?íú‹(ÈpÆ?'ÊfƒÐ€¼?|°/²·¾^?p<3!A±?¬ÁG}!ûÄ?'(¯%ÃÛ?î‡ò…`Â?Š¯ñ²Má?XÕDó—Â?M{Õ\)?¦Èf°
5¼?ŠŒéUšý¢4FGL J0232.8+2018¿á>Æ»LÀBIöã÷‹½À:S»'ˆÛÀ<Hö~vþd@!TƒêÛ«?üŽÛÐuÏ?¼"'¾¶´ˆ?'8W¾}÷?ɸ%õç?þªÿu@ž×?Þ"@œ¨AÓ?µê!ÇP0¿àÄ=ÝT¿Ô¡÷¡Œ­"¿ÚŠºÄ³¿Ìœþ¨çë6AGNbll3FGL J0232.8+20161ES 0229+200?îz…³ï€?›cVÍÖvÁ?`êË~õ ?Tsdêô‡?§IÄVˆÀ?šÎHŠ¹aÝ?ïkS7?šV(Qôt?PÊ}g)P?XýPoŞo?›eíª\?™óõ-bÍ?í4‰fÇD?—¦qï‰h?}øU5LCò?ipC!ÚþÜ?´öau£?–sc…3Î?ëVã.åNV?™âp2©à?…}Ӓ 79?q8q¥Ý@?ÁL–@Ã3?šFˆ'‹4FGL J0232.9+2608?ß<«¯æÀ?eO Ñ1À:ïj'"À<'Ù\'HC@ ¤¤ä%ƒó?ýí`Á
÷«?ÈÀ˜a
[ù?·è>˜A*?îï
'ær@=äÉás?î:¦>Ê.¿•+Êz`ª?ÁéýŠ.í~¿àœ~á\{׿ßµQ†'¿áhÖÏ)žAGNbll3FGL J0232.9+2606B2 0230+25?îï4E2?œ4˜ê#ìf?Pnª¼É$ß?Bª_*ý? ‰IX%c¿?œ÷Î'?ïJœë?–¦µo$vŽ?RÃï4Q(Ñ?\Ú£ÇÊiÞ?œJm‹=‹©?–XX¨a¹?îö"(àê?EªPwiò?sMÛ%­v?a¨"Š?ˆ?¬fÜ\Í;©?‹ká³H«?ívÀä{+Ñ?'õ֒ÌLV?z¸0¦BŽ?jíw­Pú?²žw	=V?'–Ešhå4FGL J0233.0+3740?îñá½'pæÀ4ñÁç–|¯À:ç±m˵vÀ<£¦Ç…ò@˜AÖd%D@‰cՒn?Ábǵá£É?ƒ:5ØeC?Ãþv½÷qç@'3úý?ïüp(‡Ç?"AØp!¯¿äÎZÁlœ`¿âü¯ég7¿ÜXRݦ)¿ÝDÉޅÜÎAGNbcuNVSS J023308+374201?ïâñïb-?d­Auà›1?@
ÆÄÿÞ?RӐ‹#?i7_k?`—¯áÝ!?ïÀè©fú
?~ù¥0/€y?" ³…œ¢?5ÊïÞ?Ã?~úÖFæÍå?~E)Ò½?îÖ†OŽ?†T0ãÛӅ?gèwÜÅá?XLˆ"«[?¡%y‰Qÿ?…E³ÅÿöX?ïùNgù?p晆\é‰?VgŸýñ%?GFЩ('?‰òM¬§ÜÒ?p§äDQP?4FGL J0233.5+0654?ç‡Y'à´ÀGøAþ¨,À9Ì$$¢v¸À<8 ŸGX"@þL'¸€@®ÓØYÈÉ?±.Ù\R;¿}éHi·dí?ljÂáçf@
GU6hG?ÄÜNŠ|›1¿ã>åD'׿äÉ)¿—>¿éú)Çy¦µ¿Ñ°Zü$ÿ¿Üw¹à`þHAGNbcu3FGL J0232.6+0646TXS 0230+067?ï_3ŊÏ?âù±2¹?M]Í!£ÁÄ?FþòóDëè?".˜å¯(?‡ôÌ8?ïÅ"5v¦?>Ü,;2?"_Š¶ô
?8–7gVBì?|áº&õf?€Ò¶ éš;?îÁV¸'Qþ?ŽÚú"‹?kã4?qaZ?`Ž7åÝþæ?¢,a9"É÷?©%.Ëü?ïÊtÅsJ'?cw^ S½?<Äq´—ÔÛ?1¹Qã!/	?xùV+AÐ?bÝÜ+̦4FGL J0233.9+8041?±.@VZ M@2­‹`ñ²_À;X¯ð3íÀ<Ïoì÷å@"Ď_|½?ô'ß(#½?ÒÜëû?ÐÄ C?ùƒš¤["{@ªM¤x›?ïù9r•T¿èº'S¸¿ïbË#/°?ë©b>älQ¿à°Ã¢ÆO?Àš2›³¥4AGNbcu1RXS J023428.6+804341?îù×£§ð?®yÚ¦÷•?~=	Xù¤?¬ÀCjêÖà?™>¼HɃ‹?•)éô5/Ž?îC™Ñdš®?´î}êÕ"?láÃ=–?£`•q³‰?©øR9ª!E?´—'œ?ì§Àèç ?žg"?‡â"{œ²?~#ùƒ°
?·Å¦PE0µ?›·ùÔÃè$?ìºÍ‡Ù°½?§êü‰¿·?ƒéᰑiâ?ŒÒÀs¥??·¬W‹ Lá?§yQ¥¹å4FGL J0234.3-0628?³fviX­ÀM?À	oëÀ:š±§­YÀ<~Ûúg9Ë@ f'úÅÙi?ýN$Öyù?Á´-¼åN?±6ªy?ìÂ7åÒ?úÕAX:?ÐÑ`ûmt"?É
É݄*¿×—?!S¿Ûü›KŽ¿ÜÅ%Ä4ͽ¿éŠýtŠkAGNbll3FGL J0234.2-0629SDSS J023410.30-062825.7?ïŲX¥[?Š…3 ŸÇ?Y¾"-k›å?M–'³OÑÚ?œ+g'šê?‰æ¸*m—ë?ïNþ~^D
?"SE¶ö8<?RÿâòKo¸?^Ÿ®ã§ç?"ð2Ç×?"\ËÆ*?ííPÒ_±?'\"¹é?x-š€ñ?c—do~"?®%?œ:½?ÉA¤P?ìFÆ>*úú?"«œÙÚ¹?ˆÆ—c¡K÷?sô…ÃZ?º°û"3þ¦?"[ùNàÁp4FGL J0235.6-2939?æI¢O9"ÀPÀØì•ÀÀ; ìy:~À<Ä(Ï,"ž@þ™&F|@~¡ñ?¸''™z¿¼'å XO¢@9µ/ê©@5¬(½c¿ÌéìjÕ·¿é8ÝA90M¿åÆ×ÀEÕͿب'n¯¶¿á ˜%ü¿¥ 6@Ù¹ðAGNbllPHL 1389?ï|_˾¦?®PUj?Y :ù_æ9?T@Þ©ëßD?Ä±0¡?®Rlï1h?n>ͬ?Ž&ã4Ðÿ¾?D
3 ×.r?UO·@l¦(?‰ÓÑ>?"4?ŒŠc'¶ü?î«m†!.?'8(çÞ?tܵ9`?gýÜõŠP?«ÂMöÁ?'!_£I–;?î÷—Tœ4?ŒG+®3î?_l"°J°€?Uf²ÏzWC?ŸTgÎO?ŒN]õ¶‰4FGL J0236.8-6136?ì…2Òú]ÀI¥`Z³«À9&u =)À<\·ã0¼`@âô©	Ï@ž~Û¨1ã?¥3£E"à?¢gÿÚ$?ôŒ]VlG@³O؀Š¿Ú{?¼X‹\¿à.¾#¼«¿çy!¿mh¹¿á ð¥ïé2¿è%ìIiÖ¿çêªcyAGNfsrq3FGL J0236.7-6136PKS 0235-618?ï藤<0=?a¸N×ð?&Y53¾‡4?!Nèý¿ku?fÈp"Ú
?a;s.®îñ?ïØÚ²x~?zLÞKö?*<†Qý´?Ev,þ=—?rÁµ0Ø?y.'Œƒ›Ø?ïAƒš¶Ù?~Q͐ŸÏ?c¥›b9t"?V¯ŸAŒ5?•ZÙPÁö5?~"ÓÝÓà€?ïÿCÃ-7l?b;9§Ì>åÄgü­yG>â9Ì°s]?Ï
Y|µÈ?•'°'f4FGL J0237.1-0714¿î‡DæA›‰ÀMY>_· À;«ïÌñÀ<×µ?èM\@!ÁŠN"
?ú-½qåö?ՔŒ¿kG?È`:Ó:¥?ó.a«ì@ÁÞtj
5?áîÜ÷½;_¿ËK|Öt+?Ö6¾£>^
?Ú7D9ë´¿ß•ë/³L¿Ù±ž6ò…AGNbcuSDSS J023700.77-071307.3?ï5x°¶Ü?•Mjk(Ì?Y¡<«»?RV~L¾ÞÒ?—¶Ö2wÈÁ?"Ô®cdß?ï¡¡äž'?b!ú/V˜?F_N"™?W2|'Eg?Ž¶!'÷]?È‰"~dž?íÌoíÈ'$?'í ]X'?uÛîó鬳?h`tS1à?°>Á¢€,?'ì"Ù?îCJé	t¼?˜ŽØ‰'Ü?Vcýᅫ?Ql\•ÛÁ©?«æOy6H?˜'îpØ{4FGL J0237.3+2000¿îQm=p"þÀB,{5*"8À:úK‡½ÏÀ<x篷é@ [' NT@úŸ{Zê1?Ä×	&Db[¿v"ÞÖ¥ï?ªq)Ò?ÿÙ¨'{ïæ¿ê†_ô‡Q?¤¥b5æR¿æ;Z^›@ä¿ÚOõ^f¿ía@"ð'?ãT|YóAGNbllNVSS J023720+200033?îՆÉD?ß›\"±×?\ŸDtÔ?WÚÝϹ÷?¡ÂšÎ¤h?5d6oº–?îöÏSGö?š?FW±ÿš?V®5Uó'$?d9hIœ-?Ÿ»2JÉ?™j "PíZ?í/XzXÁR?›,ä(?ˆ^bA-K?}»ë¦"
?³yoåRê?˜X×v$"'?í…QœÙì3?—$[M?v2…Ú=÷?h×Q<'?²s¯ðÒúƒ?–f†PŸ
4FGL J0237.6-3602¿æèïêÖo…ÀPq¬ÄÀ: mÉ17À<}Ötì;'@ ]€‰¨4è?ü²›É?¾a"ðg‡?¦_
ã™ÿ?ér\©NBƒ@
'r—Í?êíý¬i¿æ¯2BGx:¿¹ÐÔÄ=F¿Ü®}†¸–¿äú•þ¦~?M/]»œúAGNbll3FGL J0237.5-3603RBS 0334?ïáL?ãîÐ?oïXŒÊ×?0É!kÞS®?@ø¬#OUy?lš›î•fG?l
ÕdëÔ?ï°1c4X?‡C±'s\ÿ?1#Xìa?EQ«z ›?ƒjŽ "•N?†¸ö+vŸj?ï
x#Œ?|åѼˆr?bö'ä)?Z 1!†?›ò-‰lc+?€ƒ3›M+?ï*{…ÝmÍ?{÷þ=`
«?Kºm‹I?<ºÓbÈÌ?™Ò»×÷ý€?{¬Óu«è4FGL J0237.6+0923?s>ŒoJÀF¨ÁTɅðÀ:XœóÀ<U¹}d¯­@Ij¸…˜@ù½ƒƒ­Ÿ?ÌÆôE·š6?ÆF‹?8Ð?üÙíçχ'@…Öf(¨ì¿£Mʟ\7u¿æ‡uÀ –ù¿á¡Ü>ñ§¿ãB–³5L¿èÁYAºµ¿ï÷yHÁ9òAGNbcuOD 58?î³o™@%U?˜Ô­@8ò‰?sís¶Ù +?lŸŽc?¢KWõ"†­?—YgÚ?ï*:ìKCk?™`ÆÏsg*?M·ŽÞQ?Zrøñb¼?™ÊéÊ&ÓÒ?˜õ…Ãoù›?îr3Ìñ¨m?µ­1œ¹?x‹i+U£?md)Ësk?¥ÙÑÃÀŠ?Œ*ìK¡?îe(_H-?…³ÐE¯<?g["kßK¸?S.¢íÈö?¨7½ÃMˆ{?…jýkyÇ4FGL J0237.7+0206?Ӊßc
§šÀI'•þÚfÀ;5‰+L"À<±&9O¬æ@µY5¦U@—?úÁҞ?ϵ8ªå?º=»aëW|?íUӌÚn?ÿ"Üj ¿ïÿMR™*?ïüˆFŠþÌ¿êó_s-F¿—Oé¢E¬¿å©Ÿ÷Ó¿ïÿú Âî'AGNrdgPKS 0235+017?ïÞ1P'gZ?j'A¶'Þ?0ÔOÛ¼³?)ƒ}¢Ñé]?o´%Œ½/H?i€f¤üÐ?ƒÌŽ?Œså)¤C?=	qY¨?RU¢5ƒ?‹*"\#b?‹9zÔkm?îýL̓?'eeE6òA?uhw7ïx?cŽŽIðDá?«ƒL8ß3?|J—¼?ï0°DªZÚ?'Œ	—ž??o×V?þÒ|?då¸ÖÒ=¬?•ï¢´ÊŠ?€b\þ¤_ø4FGL J0237.8+2848?ÎêYãÔ®ÌÀ<†E^®âÀ6âб§­À;<éõÒ@÷÷ÈÎæ@«9²©5?‹æ©¸ËŽ?¶NêÆÝÊ@(=îVŠPP@!%U¬ÿi¿Î¾üÀ'a¿àkÀ]RÁn¿åß:Wꢡ¿äp°×£Àd¿è6c¿Bµ¿í(/~ȲâAGNFSRQ3FGL J0237.9+28484C +28.07?ïÔžûhÇ?wvàß횚?K¿¿Çr~H?Hk¢(@µ?†ÎÜD®¦u?võbÈyþò?ï^ö'êÒ"?˜Ä$xï¹_?`mÒ|fÆ?u'§\Ÿ]÷?'ssé÷?—€Ö»¬‹?ï²h†—Ð?'A•‰½7?p$à€fè?Š¦¾su?Žã@ýÙ¤ê?'¤¶"\¿F?ï㌑ &¶?cÞk˽£?C¡Éá÷…?Cs¨ìï<?gŠüg[iƒ?aPóŸ"ÀÅ4FGL J0238.1-3905¿ï¡m$_uÀP2ñVIÀ:B´½âN>À<Š7Âäì@Ój™üÀÛ?þÛ¬´('?º9@‡Y¦?ªŸbM–Ñ?ò'í"Ó8ø@!O0ï?ÛàÈâÝZd¿Þ"›Ãjxo¿áxkì¸$Ÿ¿ÙáN¹÷¿ånß{ûùá¿Ñ顙Ã5AGNbll3FGL J0238.3-39041RXS J023800.5-390505?ïéVb¨¦m?Y¬!I¦?/‰pER­*?"}žZXR?d±Sg'?Xiª£'w?ïÇA0m?€œ^Ê×6?(Ÿ¬œ½0?AéжÎ?{šj—´c?€3‹T˜
?ï@ß…Ë?w—w¢çÕ¨?c6u>£'´?N(ü}jå¥?••¡:Öo?v¤feKV?ïÛe§?pˆ2ëÉ]?N¡Ï=²d?9EcŽ¨Ä?ŠÓìD–+^?p)‡ƒÝ4FGL J0238.2+1531?îQ@h ÙÀD˜²é̸À:n­\ÄýÀ;ìg
ÑZ@)âøc!@n<c?Ê)^H4Í?Âá
6u?ø¢ê`[Šj@rK¡éõ'¿èe‰&"Ï¿Ýä8Ž¼ÆÅ¿ä
€¡{k¿ãUÌ»/¿í;	Uê`¿äËÀ}‰ÁAGNbcuCRATES J023819+153323?ï¡£¡r¢?€µ½+œöt?W)î䌢?PÓö(\)A?"¶ZÙÆÆ?àßè\¶?ï´ªȹ?ƒŸEmqg?,æMÍÙD?E³Ô:%>?'aàÙf?ƒ'†9á?íþš'T•?žÀ{L>S?ŽéóhfßG?'o%š‰'È?´ÌÁ¸o?›
Š¤´Ù?ïW
—?¨ç?xÝDTÉ?J‡ùݜ´?>ÓÃJ?"Jà;ö+?x˜I´ü¬+4FGL J0238.4-3116¿ïÂr·¤êÀP•gÊêt~À9/f±%À;êmÀÍ»	@­ÙY"0,?ý0qLsv?§×Q
3µ¿kä#ü'?Ê]ÜT)@È/¨d7¸¿Ò¿º•'£Ü¿Ü.ò£¡¿Ü!HO$+¿Ú¤Š£ÝjT¿ßß­Ácã¿Å¡gÄ4w×AGNbll3FGL J0238.4-31171RXS J023832.6-311658?ïì%R^Qt?Z°"Q:Õ¯? #׎¯?ŒÒM5_q?bÙëp`?Yýª¬ý%|?ïÔ¯Ö'I¡?|ä¯ӎã?)ÿ6ŠýòÆ?KÿSnl‹…?tØ8?_?{ÜÁ¦m}?îì¹RGj€?ˆ±|
Rü?i¾¼†Ÿ?b6
å_µb?ŸFý߁Ü
?†Å{â·ò?ï6Þ)?Ö?xx.ږ@æ?<x«KCXi?0á"^_/?NƒUïž?xõdŸ4FGL J0238.6+1637?¬¾\ÀC}'Ó"À7¤l[ríÀ:þm'JÈ@(ôï֒@·{|x £?f÷'`¹v?·‰.'dœ@(æOTÑé@!#…k9_¿Àòèn¿Ý;'¢‡(ÿ¿ã7GpxŽ¿âVûŸs"a¿çñ=Å]m¿çÇFê AGNBLL3FGL J0238.6+1636PKS 0235+164?ï¥íƙÞ?x÷vb•Í?D*ytîÁs?Ct
Ë)EØ?…AæÂ9'Ñ?w¿[ÚêÉ?ïY…Ç-\?—.'³ß`Ò?^áv'p­?€'ìécL²?'á6òý}¦?"Y?£Š¹?î9ç'î÷?žÝQo\?"…$†FçÅ?—…´	€¿?¥ÉÏC½œŸ?˜üΛ-?﹀æàK?w£•à ùh?F¨…Ÿ¼·?G(¶:lV?€?»Æ½ñn?v‡Û'N‡È4FGL J0238.7+2555?í_#=>FÀ>üú½ ßßÀ;ÙÛ©¢À<…'e²@!!þ}sô?ÿ¤óÕORN?»äY€¿¤•Às"?ãI›árv@üó€À¯³?ïþvÞ-È:¿ëÃ<?ÌHÿä>>I竿䊗hfñ§¿ÏYm3࿦K_
7ÎAGNbll3FGL J0239.0+2555NVSS J023853+255407?ï4Ã1¥«R?'âsÕP˜¨?G½yeMéÿ??Eì¨{¼?˜©® &8?'Ÿ›ÑrEZ?îô•¨5½Š?šLgüâúî?Y!jF¤è©?c4Æò©'ç?ŸÛ4TÞL?™b3(ÒS•?í»¯9ü?–ü™¥Ñ—{?rpâ_ùØ?a;¹F%×q?²Û'`0y?–ž¼ª8ž?ëâLÝ•|?¥Ö¤Ně?pgð®
f?j?ãóm(®?¿ç£Cv?¦QˆÂ]4FGL J0239.5+1326¿áFòÄÇßlÀDØ΢âaÀ:ú–xHÀ<là‡"´@û-8¦?ÿâZµX<?Ñ´`YÜë(?Ç#–=áã?óV]Ú¦ª@žÃmþ`C?íñ'QS…¿în16ñL?Æ2ØÅS†»¿áô²YƒÿÔ¿ïÿæ¦Sf?ïþùÛ"ÐåAGNbcu3FGL J0239.4+1326GB6 J0239+1327?ï«åšÌ?"öq‡r¢?QÀ¢ÕfÔ?qF(/ì(?'ΪIOß?'ŽÞ(Ÿ3ê?ïb¦s"¥?"¹|DôF~?H 	TÆVE?`ýacÂ,È?'æ1TÇXà?"–ì4ûs?í†Ñ4õaî?‹øŸ%þP?‡I­>B×?'"=PXÔ?°àVB­(8?›tÜrÔp°?ïj‹…/?~ŒÈïI
?1‹Gû\(?+>W|!?'yoo‰Ž?~Cë_ü4FGL J0239.5-1353¿áúK±6÷ÁÀNÃ3ÁÎl	À;sýþžÀ<we'+@¦œ%.@œløPß?Ƭڝwö¿« 8Bf­?ã#û½{ 2@Ý»´MпÓ
e@¡†¿ë䩘^\¿æÏ€Ü3r¿âf="†¿ïL_ŸLáÛ¿îµ{aöDAGNbcuCRATES J023939.13-135409.6?ïÏu†GŠ?tåóÃä?aoã•,?a–Vm–c?o–#iÿ$?pŸ¦8
­?b•àd?ŽtIš×F?Kì•àà7 ?^×Xš¡â¼?‹]üyãÔ?ŒTyÈÊa?î6՛ó@?ÈToJ?{ßÞËfæ0?p²VÙf~©?©#ÌÓï0?‹úl‡Gc?ï­:͏­Î?q!®RO?WGd9¢Xl?M¥!!Ÿí	?È`àA?pšS@Îj4FGL J0239.7+0415¿íҚðfÛÀH'øã¬cÀ9ƒÇhß½jÀ<4Dé>›@~UñN6@ô±$Йá?±Š*!!ôÙ?°ÃʀÓ`K?ö‡‰	ÿ]@_Ÿ —$I¿ÄE¤¤å}¿èTKç_J¿éó¦öyn¿æûÖƒó?¿ïþ©žttÇ¿ïßÂð|AGNfsrqPKS 0237+040?ïûzÍ.¹?DX}²ø?*ZL)­ã?3ËËôü¼?:wpu^u?9µrãQ%Ö?ïÄþ¤¢x?ƒIM&¥Å?3æÒlî™ù?U1!ûãó?|Á†ßÚX?Òàïò¬?ï?G~žý?}J×>­?mŽ
7ßQ"?`úÒð¡uÏ?"^i06&?z}3(<ÝB?ïïœCÿ<;?OCÚ͊?;£×ÕK±?4Þu5¥?YނCõ}?J:©G4FGL J0240.8-3401¿í¤'I'LÀPcˆ†aÀ:øg³À<À–Î
>­@ó"¡ëx@œˆFŠþÌ?¿'t Õ'Ü¿¬lB|?îMâÔv?þ/r†r¿â0'9¿äC#k?;¿åsþwY¿âö?ç̂¿ÜtßzúG.¿Ü䜢7£AGNbcuNVSS J024047-340018?ïRÉû
Ç?Œ¾k,Yµ?b|±3Fé¿?VÃãu7ä?"W*vÕj?‹@ËYˆ?ïg0S¨R?'°ú}ãŸ?N߉Ì*áÕ?[F@À=û?'"ùQIž?Ýi´Õ›?îCÞC?ŽÂµ»»?{‰ò«¦á?j	 ˜rí+?«Xñ\§?ŒW'ÐÎ?î´A<üñ?‹ Ém?j??hl.ÓÓ·'?^õæê	KP?£5)R'õt?Š´24FGL J0241.0-0505¿Ã3k–•ÇíÀKìØ]ú‡À:±²dkºcÀ<'£¤µW@µ×‡eåb@]OG"=?ÅAæ0 .?Á±Ï…ä°ï?ú\œÓà½E?ÿÈaMw×þ¿ï˜?ǖ,'?îóÕðaýK¿Ýá,Ö!à%¿â2ƒ
¿ä:"DÇ¿ânA§VAGNbllPKS 0238-052?îæ
˜l4o?²ÃJ=å/?†÷äá|?²V¤X$.?˜4±cˆ?–S`IÌÙ?ïÇï^.õ?˜©–ôÌZ¡?f¸ÌíO‡8?p§'°å"È?œèv0‰?–!B̀*È?íû'¶ƒ2Ý?'³Í`Œî¦?~/€‹6º6?pûëÏÉ\µ?¬‡"†eúè?ÅŸÖ™iÉ?íЫÞAl†?GªÚ¥½?‹÷½Ó²óž?x‡"*{j?«÷R¦üz¥?/'Æg­4FGL J0241.3+6543¿Ø"Hsü@éh=;À93?Æ¿l'À;˯bXº¬@ 	G…z¨¾@°Ê1u?°‹lÛ Ú?£^î^(:˜?ót‰Y°u~@áj5¨ÙS?ìtxwàâ¿Î´
^'ӄ¿á`¢' *¿á'æ™ýl¨¿á׆߭¥¿â9LÝ~JßAGNbll3FGL J0241.3+6542TXS 0237+655?é}XiÛ²?²'K^J?vÔv÷Um?jc}
×?ÉS*' Ö?±ùÙ!ÃÏÞ?æÏ4ñNDÆ?ča´@?}¥ø¾Æ.?‹7ù8‹ÿ?Ñêþ={Z?Ä9•~?ë©xÊ¡Ðo?£ËwB:Ì^?ˆ´–¢=±°?vÃcBk?¿¦Ö©ÆZ?¢£"
?ê$—וîÐ?¡…ÈgðÇl?£Ý"—o5?‰·e°æ?Âv;»Ì}s?Ÿ.º$хZ4FGL J0241.9-1603?ìh\IÏNTÀOýüÁrÀ:Õ¦Zr<À<'æ$Œ§C@ Æ*uIƒ,?ù²¶»éOº?ÑmÝÞÂî}?Ãñ¢õŽ?ú4°%Í#@(·'㟢¿ïþ"ÖúÎ?ïÿ×hE¿çånÿ½¿¦qì™­ç¿Öý€^_0è¿ê³Ù¡FŒ+AGNbcu1RXS J024151.6-160339?ïÊôŠgÝ?r:©U9Z?C2²lUŽh?=µé&ª?x¯mA_ñ?qîÎr¶"?ï¾2ڗª?ƒ-þH?6rã.ñÛ ?LÐNLòÄ?¸_Å
Q?'ac™PE?íÿ¾>Ãvú? ÚB
-?r¦ÁÜ|â"?déö!"Ž)?­¯CØ8ô%?›Ç£Eó?îên>r?†*šX¬?]}`¿Äk?U' ^Rm¥? r¾áê?†
Šn!–%4FGL J0242.3+1102?†ï[Ð'¤ÀE¥ÄڐïÀ9¾½¨!óÀ<1Š¼‡@X:þُS@{ÇÜ£¦?ºýT)"
F?Ï+WÝ´>@Έ°=@$'w=N?¿Óh'cëý¿â¤ðñ5¿æ¾ð֗Pê¿êðþÊô¿ïù•¸c‰<?Ú6†¤ÊAGNfsrq3FGL J0242.3+1059OD 166?	e¦O?šJ]¿, ?xC¢›ø?ˆÈ©ò*@?|ûY2;'?'Ï=HÏ?ï6‹º×Tü?œcÅ!
C—?\AH"…?p3Lڒ¯7?—jtÍ»?šG'¬¢7?íiŸ¸—÷?¢2<—|g?£ŸU0œ0?•¢ÔºNi?¬BƯEäQ?–héÿŠ1?ïwñ§àÞ§?vž¿úJÝ~?`,g
Zé?O+'2Ýí?ør®¿^?u XA‰>S4FGL J0242.3+5216?É;XŸîPÀÚñˉ֮À9mmþ
\zÀ;²'쮤@3éހ~@_°&£Ø¸?¾ÁCכ1õ?˨]ס'@VùzªÁ@²¨ÑÅÛ?ïÿn	È֞¿ß"]ó%Q¿éßø…–W¿è,ñÀw)¿íA"d~.Ú¿ïóãðµAGNbcuTXS 0239+520?ïUÌá½ß?•JP¦Çðè?¸o©ÔÚ?`Ö´"ÔÇ?•9ŽÞ@Ô?‹þ!JE]?ëLôÖ`ïw?ÂÚÔ¤þ¼@?q‹ßŽ wÝ?¹B*Ï-?Â?ͪ>g?Â¥JnƒÇê?ì>s-'Vˆ? ÄèìRZ?¡N\hVQ?²"à*?µe8_㠚?™Iö¼‹?í»ûµ¼ß÷?‰ÛZïº?•ŸçÀëÒ$?ECafk?©pPüv?‡¦"=•84FGL J0242.6+1735?ï蕉OۜÀBã4›èÿ2À:8.©`¶úÀ<-V@½XÛ@y÷šÖ°{?ÐÿR©úe?Ö‰bÙ?þåä`gHä@;ݹ"¬?ʲî)hÚ	¿Ö¸Éà‰B4¿á^'ျ¿åQ)=f¿íî6ߐð¿ß¡¸¡òƒ–AGNbcuNVSS J024248+173700?íœváœjr?±™Ïɔ?wûhT‰¬ž?u€ÖRd?±œ'mԝ?°@[¼2Ã?ïõSÇ%Æ?™ûz_Ï>0?b²kžCñ?qÖÙuÏl?›«9§~Ã?—ªŸúe?çªG¶†x?­Y~iuX?·ßÙ_E‰U?ž¶å¾0?Åf÷Eƒ!s?¦Ñqå­nš?ݫñ­?"ùÿ%"
?qüÎ÷v…‡?_ùœd'?¥(FR?ƒßX¤•4FGL J0242.9+0045¿Ã¡cꂌ¯ÀI¨	ÃÎ ŠÀ;;éÿãzŽÀ<¤§:l™@±)Î/£?ÿÚ¹šû?ҏ¡·uM?ÃjÔL?ô˜çÂòXx?úiè‹Ï×?Í$Cy|n?Í0"W=(ª¿â~Ȃ=¥¿Ì­W|Ë	¿ïÿwy´!?ïõgÉÉãAGNbllFIRST J024302.9+004627?ï'îíó Š?™™UËdø¦?l¿VAÉ+ë?˜:µíä?"Tnò¥'?~°fKÏ?î‹äz¥Ëv?¡õfЦN?s~ÁFs?€ß×Ù¶ó?¤Ñà,ßzF?žÔc¼»T?훃5=ˆ5?•ý¹ –gÉ?‹YjVÁ8?'rï(ŽÉÌ?¯qr+ÑÌO?'ø2–Ä÷à?ìsît	? ž­ßáÐ?Ša¢ÛDïª?€ÌœÞþß6?¹W ÷•?ŸÞs"1C24FGL J0243.2-0550¿ïÛ¯¥ÀKø§Å¬GÀ:Y¹'†¥¡À<aß 'á@|7ýÈBO@Æ<ÓG?½nÊc?"KtÈ~ßY?Ñ÷œ§@ @1|ª¤¿°àøûÔÍ¿éÔ¾³¯o¿êx/â縿é§ã¿³	¿ïÿúVrÓ\?ïÿânÁŒAGNfsrqPKS 0240-060?ïù;z	F?pÝÆFÜ[?/îÙ­"y?Qx»ÀvÝX?CaoŸâ?gn)W^}?ï½J‡é?‡k¨2"?:Jhðô?\a@3¾?¸ÇØ4í¦?…'"Ðk?ï*'£´Ã?ð¯·?i™'ˆHß'?WRUxôò-?—z™XsK€?€"YD­ò?ïêA¢h?Tswš%Ò¥?+7SÔ
k?!HJ8ò¤?dKý…€V½?S¡°D²$è4FGL J0243.4+7119?ï7üµC@$Ȓ‰ÚßµÀ9¡¬JvE×À;àf$ø
@Åo!JþV@-[h¢×?´˜Áò#?ª_z@ò'Ð(¡à@›ÅB궿ïýQœI?ïþI|JÔ:¿à­‹ßÙпßÖ³jû÷]¿æ"…€‡ú¶¿ämNí£ÜéAGNbll3FGL J0243.5+7119S5 0238+711?ïñÅÑRëi?V ²©‰Í??JÓŒçö?8~jp]p}?T¡¨™…óý?R¢X(¼‹?ï'éR#†€?–1mA?Mjà.cË?c x¥R¢?‰nýnKyÅ?x(¦Ÿ?î&"ï…'?"ÄLHdmÿ?_}²é
¯?xôoH¾/M?©?Ñ¢ýdv?'Ge4÷Ÿ?ïy
U±üà?t+O²W?e(¾Ršÿ1?V]ùl?Œs:þÚ!?rÀ…h$4FGL J0243.7+0321?çø"y']ØÀHœ¡ô±îÀ;V¨°ÑåÀ<¬…\ '@H.ï><@šMô™?ÔçB.x¹O?Ófæ~y­–?üõO؅g³?ù¸0—!š¿ïÕv‰Ê½?ïÿEZ}$¿âîGÜ7£Û¿Ø8OfÆ¿ïÔF"
q¿î·N: AGNbcuPKS 0241+031?ïX"Æ'é?'°rGl?rPØ('§l?p:u†Æñ_?[10ùxç?:DIv[?íröýѦ?°–›Þ¨zJ?ÿCj›Z?˜Ú~ãön&?°¯‡ÚÎj?©Ä$X4±‹?ë
~û,b?¢a÷›¨Ü?«5(vj?•J‡B±?¹"'ta¹?š*ŸÈc`"?ëSœ
åŒJ?£O‹<ƒ¯Ô?§,³{@'?˜<eÄN?¹ÌÅÓKýt? ("A4FGL J0244.6-5819¿ÙàšC&ŠÀJ‹ …±…À9º'‰)ßÍÀ<0?\6a¼@ ‹'6û"¶?ûÜ ý¦‰?±
Þoú?¦å|."£?ø‡¿|'2@
€†µ‡Œ?ïaL'HD¿á§©Ý^•b¿Ö#ø'Äj¿ÖH:	ç
¿áÈ4ˆ¿ª'_ÁåÕAGNbll3FGL J0244.8-5818RBS 0351?ïàf«€{?`õåÍað³?-'|³Cíî?¥3­_ē?mÆÜ´>F/?`h¬Ÿ¥ ?ïÈì»
Ý?{ØËy=Ï?$M($ º?7jî>™¦u?zå ¹l~?~Ïg
nV£?îïQê	à²?…Öý8þ¾Y?e¸'þZ2µ?U>Zqëã0?Ÿ^²^ø£i?…ú½iòº?ï>§™?~'hÆ?R¢¢BÒãÈ?@!Y×oRr?šî¦ò~Æ?}ì"[g©è4FGL J0244.7+1316¿ë6ϟåäÀDÍ_™Ã‹À:h¢À‰ÈkÀ<+ò£ +@¢|f-@Œ°Úþ¾·?ÔR°+¬V?ÐVMênžC?þ¼g#û‡Ë@
Wxelì¿â^lg1g¿ã5V=ú6'¿åɓAÄ¿ç?¡k2Ë¿ïÿyݼ‰3¿ïûfKŽtAGNbcuGB6 J0244+1320?ï¡0þ§Ìs?†ã™ÑkÐ?T
ÉoÕÖ?P)ü¦2?…2((¥?†1Ð鶶'?îÒÉB?  ®ý)>Þ?a2Ꙓ]]?kù×
?û¢?¡À=4–Z?ž‹Všá)m?í}ñ±ž?œ­g9·ðà?'fIySf(?…å'	͏?®óü(Dó?–ó°IÈs?îYÃyÒ¬?ŽjïÚ¦?é?d…SNˉ
?Xqç³.Q?©s-ò,Â?ÈcOŒ¯¥4FGL J0245.1-0257?î¨Ú&§‰œÀJÏohیÀ:B˝!äÀ<oNÇ
p+@ޙÙ/†«?ÿ¨×úþ8?¿uÁ"I«ñ?¾8œ(À@ý"$½@
ý
ÒÁÙ¿¸ª½¬s?ï]&š¯™¿Ó86¨¿âѤÆôF¿á4C~"ë7¿à¯3ß«v¼AGNbllPMN J0245-0255?ïó`ó ?Pa쬰u?6ݍ²x>â?2+PtÁé?TÚ­!à±?L-Ï]n
ÿ?ïËP¯žæ8?	‰¦#Q?.Õö¨´§?BÛ°e»_?yg1€×žë?}ڂ¬jŠA?ï(\Ï7–?9*Ï_4?k~g³1÷ï?e£¼!ÿ9n?—"™'rÎN?zsÒË0ÿ8?ïÀ/è5Äæ?dY"•('¹?PZ«=Ñ<?ASh¦'(â?{Ña©>?c…åá$L4FGL J0245.4-5950¿ìÅçÁÖà³ÀI÷\¿ôw6À;#£Ï}5À<ÏÓ¦Û¡|@,¸aúœ?ýQ3~²†?Ò7'ßm
u?Ó¬ œîã@1õ`iÍ#@ñ_	zÓ¿éÆk>'aí?îþQ>¶ôô¿×3ŠÜgtƒ¿Ø§¢Æ¾ì¿ê¨^=¢ø¾¿ïò'šx¼ªAGNbcuPMN J0244-5948?íÞµéa™?ȉ1.w?€ZK'ç~V?"|ó	ÚÚÕ?­þŸìŽ{?ÃmûE;´?îÞs@ÿj{?›ÎïxKÚl?eÆ=?qZeÌî+Ñ? Ç3§"Š?™m7¿ÙH·?윒P=R3?šêN	Q? !nzÏîX?‹øk›o}?³
¶@­w;?'ÿ¼;	Ù?íô"Û6f?¿ÿòP9'?‡íSlæʛ?u¾Â钳m?ªÃáçæå?ŽëO ˜·Ž4FGL J0245.4+2408¿ïmeÃ07À?ÐaAcwŸÀ9«Ut¦›
À<ÁJ¸Šö@>ÎË)´"@._#|?µtîêXùÁ?´ý"€¢6?ø'"d¦rÆ@¸øU'¬æ?ãºO¼Öµ"¿äk^R›®G¿ë¹ÒߋkY¿á²¡bÃÝ¿è"£Y5ü¿ïöŠþøïAGNfsrq3FGL J0245.4+2410B2 0242+23?ïàpWiðŽ?™ŸO	,*Ð?F‹ºM˾Ù?t SÉ7FÇ?i캜'¦?"|\³<Ãö?ïÂZÐ[ó?€/Ó¹m͗?+^[ÛÛ¤?@q¢'hPÐ?}ùüߘ&ç?jb¾DЏ?îÖ
9±?Žveê*I?px!5|û?k0Îyêç? ‹5¿QU?Œ©®fÉ^?ïÖQuù²a?^A°WT×?G¹ph"ë`?9?Žœ®?qàö"r÷?[ò¢"Ã4FGL J0245.5-4502?Üò6±,DÀN‡|í'hsÀ:Ð$qÏP5À<sóëõ‡@æ•â@÷ퟫ+'?ÄX½L&I¿°Ôí=ì°Ô?àíX]'@Z¹D.Ù¿ÂÁM½£7¿è>}i7Q¿êþdŸg¿ît¯45'²¿§".ÜÈ~›¿Ô CVìÌAGNfsrqPKS 0244-452?ïßzmZ'ù?t&X׍`ƒ?GÊ燦2?Px}+?j'ØÃî]÷?råÔ9òg?ï~Ò΍°î?"÷­+6ï?Rm)™Õñö?k™7AÐ2å?ý§)Y.?'ù%Sãd?íK(ž¬0W?™ìØ\6‹?¦Ý‹ë¿?sátҗ ?³qßY!l?˜k|¦ž%?ïË
Q"7?j^ùâ$œ?6{ªð¼@‰?5
¤àž?y	¾¨* …?i£º»€4FGL J0245.9-4650¿ßå–êŠÀNàC¢@À81Êx^¶oÀ;¿Œæ,ð#@­{MÔ@w¹Z)AB?¡™ÿÅój?½Vö†Úz4@%4z[ñ@0|o'4¿Ðnb×Vi¿ám=¾§p¿æL"üÅ¿ç}Ëb>Ž†¿éÖt€Û\³¿ìûgPAGNfsrq3FGL J0245.9-4651PKS 0244-470?ïUØÚë6?$+Cìi?hMì(Äg?eèàPPÊo?';'‡ld?ãúÀ•Î~?ï¯9C¢§?ŽX¯Yž˜?@TWûe"Ð?Rì¤R9?ƒ,iº þ8?öå_Eú?ï>Ûâ
Ìü?ˆ×nŠT?zZ™ýñ˜?xEnÍI[?'Ý>Ê ;?'Æ5²Üë?ïìºik¸?Rz†-`?2ù1b
Ù?*hÍ&­3'?a"sèk?Q*–³'¦j4FGL J0246.6-3348¿ëþ‰¼héÀP–=Ć­À;Òh;R¼À=ØL\Ïå@!«5MiÀ?ó÷ ›šœ?é£,àˆÁZ?֍˺Óûë?ë½Pù׳@¿¼§»›L?ìoè%ç}¿åú9¢8#³¿î†9[e?àçŒ Š9)¿Ö‹ 1¹6¿ãÒe}ˆAAGNbcuTXS 0244-340?îòd"¶t?¢%º,]F?e1]×µW?`¯•uى?Ÿ‰=sZµ?¡éºòUÑ?ï˜;×Èà?ŽìMžÀ'#?EÃNB‰Õ?^˜…Ö7»?ˆ"ÕYåÏÂ?Œ·FrŽ?ì'ëêÒ?¡ÜÚK[;ï?'û}TcZp?v>_þ(?¹çö>?¡#õd2`†?ï€/£Ûo?'F°wäj?$ð.á_ë?;Eµë¥{Õ?Ÿ&­ÁÒG?'D‹Q(4FGL J0248.0+2232¿ÇŽW_ý'À@r9¼º0À:ތ]pô_À<]ÏX˜GŠ@ }¼Î§îF@1jWX?ÈS¤|Ü?£ËF¡
bk?á(2F@̲-9I"¿äDÌMKn¿â՝ÖÀ¿äj‹Û¿à²Ál!'¿Éµû$#ë¿çÓû?PøÁAGNbcu1RXS J024800.1+223136?íy3º€?¨H°,C?^ñZÄ¿±?S»Çƒ>A?³»ˆ Àì?§ÅLó."?îÐ2D¼Ýb?¢%w8È®?W• äbu?pLö+ki–?¢@.­?¡j]¿C$?íNàvR?˜\x¨?s©;ô¡º*?_ï]ª+žF?´NhóS‹?—¬jBÅ©¯?쑇Êûâ?›†Ïº]ÒÄ?a­fyÂ×(?Vþäa¶ýŒ?ºæVtRÙ?›ª#¾!¸4FGL J0248.6+5131¿êñ>ÏðÀçX}o—hÀ9NÎþÖ4UÀ;ÎDŽŽoš@N°A¦¾p?üçC:è3[?³YP¢"Ð?ÀÌê(þ&@©NBƒ2O@OZTŠEê¿á©åan/¿ãQzç&ë&¿ßÇRÅ؈¿ÖÔµÏZEÇ¿à=ÁA(iV¿éÊKéžtAGNbcu3FGL J0248.4+5130WN B0245.0+5118?è-"¬†?¶këƒ#Sw?"P܁¿??‹XCc?Í.!|?µ]/kŸú%?à³8pûe?Ëy[–1¡?»P¬?¡›±Ï.K?ݛ³n˜¨§?ÊQ}uÎi¾?逮owhM?¨Xô‡Ca–?¢¤¼FÂ0?'‡ñ?ÅvÝ®??¥ ãÿíb{?æ"m\FìÈ?©÷	9=?œ:`äâ-³?†3±9E?Ñ÷9$"?¨ÍAvwl4FGL J0250.2-8224¿ïû;>^NYÀ@Ӗ¿Ê…ËÀ9Ô	:;e1À<K›•ó@ŒGœÌ©ç@ÜÈÞ*Ã"?·'Ž zÚù?¯Åìûw?ó«TA ´@@ŸÇ™‡%#¿ÖÌ`it¿æõ®j}¿æIRŸ48A¿êA<ÀûˆL¿ëM'Ÿ'ç¿ïîxžwNìAGNbcu3FGL J0244.4-8224PMN J0251-8226?ïæVo÷î?…̉ºFJÔ?0i#«6­?Lú£S#"?gœÄ/òª€?"KæI_Ì?ﺍ†»Ý?ƒ¤	¿¯?0›Æõr5*?Q¬ˆ[ùª?€×ÀC¥võ?'K^§_€?îù‹O	´?ùáø‰<?o¸ª;¹?f7"(xÖb?œëÙ×gÇ?`ÛP }?ïáX_?rz?Z/}}Ÿ+€?@-+
¬?1f3L®Îf?jœUÙJ:?XLGÑø'4FGL J0250.6+1712¿æ¾cݗl»ÀB‰‹`ñ²_À:àϹWÀ<*v­ÜF½@ ´¹‹Q'T?üB # –x?¼H%)Û?®Ÿ
át=ƒ?òÈ¥‹?cÃ@Ë:¦o¿ÓÏ"'|¿å¨HÞì	(¿Þ'1£X¿Ô¯$f‰¿á™Ÿ]þ¸Ø¿ÓyA쉁AGNbll3FGL J0250.6+1713RGB J0250+172?ïÄv~–Å?qKƒõÿk?9øÛÏw?.© zCó?|%?vp­?pÓ%÷Ä¡?ïw°Ä[?'J"åo«?>	û9sš&?N¾Sàúk?'¿‡¹Oo?'(€yœÎÊ?îê­ÂOŽ1?…<…†³ù[?e¡9ºFë?R¥FWµ»? )Çkxu?"\L(›?î Ö¦çÏ?Œ²ü7 ½?_[ô¤‡Ëj?L°aW»BF?®óðmDÄ?ŒJ49wUµ4FGL J0250.6+8435?ïŠßŽ_BŸ@6ir%·I®À:	L‰EŽ€À<~ÿÕ7ÕY@zR½'¾?ÿ¾Ø»gJ?½{ ¡yüŠ?¹íߨ,ì?ý<<& ûù@ð"W_´?Ë©©\/UÙ¿áe'¢xæ¿ã¨üþÿ޿כ#¿äÆ÷ µî¿ïÿ
!ANAGNbcu3FGL J0249.1+8438WN B0239.6+8423?ïåè2¼0?Yň"Žû?F¼ƒD²iê?<Ƶ¹ƒó?dhNü5F?UŽ­:00?ï)ÈÖTŠ?Š©¬8U?]&ÖÐ,Ðä?i{qØîxÚ?Œ²ðeC5?†Ò¯ÐHÕ?îñ-úÓN–?'IJñ¤3?p>Q×'Þ°?dÈ \MÃ?Ê¬/Ì5²?€Î?%R°?îóÀ¦"·?}tCk%¸?†^{û[§[?kópv¼|?–_	í•ž?wтÚthZ4FGL J0250.7+5630?ém<«å"ÀíÊ"Îa"À9ÙÓr²À;çÙÉ4'Ø@ ˜ù(öCi@Büý@´?¾2ÿܙžw?¡]¡à~Ê$?á/¯4_?ôlÃk$;¿çë«_>ÔÒ¿Ûï—<M¿ã'#? )¿Ö2£uæa¿â{ÒÿkÛp¿ä	•ª÷ïAGNbcu3FGL J0250.6+5630RX J0250.7+5629?é¦ÓjN‹?´ÂßÍnTê?zõH:Uâ?sCÉ»Øçß?ȍó$ª?´›ƒ(ã[?×ÐØF«§%?ÇÑ÷	B?€®oO<?ŠZÍQђŽ?ã×a$<o1?ǧÛã ?ç7€dlÑ?«Å¦›,Ëx?›\¿Ù)ˆ?çfV°/	?Ï¿ús'Œ?©ÓüÈ5±‰?ãU•à!©•?®Ï‹¼{''?¯Ë¶«ô.?™ÅDê|8Ø?Õ[]j>)±?®Fi—ž:4FGL J0251.5-5958¿î½ÆaΧÀI¥£3vOÀ:ËGxd•¬À<»É{´Ú@øTD«@ÁÅàIS?Ç)%=QD@?ÃzO|jÝ?ùͼì"øù@

yæ ¿çOÊB®Ñ9¿åm÷T_Ó¥¿Þz&ÂaŽæ¿á°.fDØw¿æŽ"¬Ï¿ïÿ¤?åÉAGNfsrq3FGL J0251.5-5959PKS 0250-602?ïêÉä´Í?ap8-Â>?>{×¾ß[?Bx~åã…?a »#oF°?^=J7œ€f?ï‡èyÆ+§?öF·ÁŠ?;Bv9e?Rš
ԈV?+ÐÒÄd?c®ÕL‹?ï °?ƒ"'®±i?j‰o²ì·¤?d¡Í2pK?œ-Î
?âÿNYÒ,?ïƒýoz›%?v¡)ÄÃ[?MOäqÝV?<ó©ùG?+¥Ú;a™?v^¢½Oì4FGL J0252.8-2219¿ç‰ ­ŠfÀO£n.²À7ÐUÑì"À;¾t{'H@²«Yà@òþ½x?"Ð-'Å?¶փ¯Íc@ãrý›¢@XxPô4¿ÅÖSeª)¿áãА俿å¯>Õ'å¿æ—cÉÓô¿èâ­[µ³¿êªàHª"½AGNfsrq3FGL J0252.8-2218PKS 0250-225?ïl,ìÂQ?ˆU¼Îûp+?b,Ëҗ	‹?]sg³õnó?4ÈíbìÔ?‡4$ˆRÕ¶?ï£&T"kØ?'—°Ì?EE²3Q!?VúýÊæ?…â²!Ôë?'Km&K?ïQbr¨ŸÃ?…ÈØÝêË?wJÍl³Œ!?vÔ¬ü­žÌ?þO¿$†?'-/O¶?ïö&Ö9?Dä‰ì¾<)?)¿ »Ã²/?&ÒUlÔç%?P·Î<Uü?Bq©vdR4FGL J0252.9+3834¿ïÝê)L;À2ipÅdùÀ:[>¢Òþ?À<YNÛʗ@Ïa&
««@%Ä'â?Æ"?ÃYí\9fÔ?öȍ$@Q@àÃA]ÃU¿á¤1£:á¿ä´|ÿ…ä¿èE¢>Ù°¿è3ªÇÜ£¿æuI"ˆÁ¿ïñ$€	AGNfsrq3FGL J0252.3+3830B2 0249+38?ïgŽÏÂð‹?‰{ýYÑfP?`57ãÄbÿ?[U	¨ñË?')bE?ˆ;ˆšº?ï1> –©"?žä¡0Áú?];ÚÔÊs?l•è>?ĺ?˜ƒï}€Ù?;ÜöÊ?íð…=Ñ?—Ù2pUÆ?~ÅÚðèçÐ?qŸi̯bŠ?­óA_õ?•—éw2Œ?îöù܊@¦?'%
èR?qJWȋÄn?[WtXãK?œÎ.|"ùó?€ï‰¼ìÜ4FGL J0253.2-5441¿æ'
Ê ¨ ÀKR.±Ä2ÊÀ9®æb IÀ<†Õ™úèi@È܏ú‰@åZ'"Ã?°uuøՔG?°óéœ;_}?ø=Žkh-ç@¯³ÏzÒ¿ÛN0¥lÕ¿árç]ò¤x¿ç»e4Ù¿éIiÀãàe¿æÇ>îRX'¿à÷ÍaGBµAGNfsrq3FGL J0253.1-5438PKS 0252-549?ïé¦Þyˆ²?d~¹@µÈ?#þâwÇ'ð?…ö"*^?e3^úÜ?dCJ9Êz?ïÖÄRý6¤?|½ï^"í?"="@'Ìk?:>"Ú§¡Q?tíocp¥?{>B3K¨?ï5
ÂÌàq?~÷2–[q?fîlâ:Ó¨?SL˜Š ¢?–€Ú
—c?|Ò]NÖ$Í?ïùd±õáâ?8wÏOÔ&3?>ÏwOé?,ž\Ê?F…f.‰Œ)?6Íôx4FGL J0253.2-0124?æµ´Z@ÀI‹Z ÝÆÀ:s­<
ÍHÀ<xåÕ²Nœ@׫¤^º@X¿ÜúAz?¾1Ò55?ž•AÆü?â^˜?ü4'g"#?焝=èîÁ¿ÀÆïh-:÷¿â·#\=¿à"Ñ~7hw¿ä	ˆ>þB'¿Ñ6¯ÿâxÜAGNbll3FGL J0253.0-0125FBQS J0253-0124?îÿüpp|¾?­É'ô÷?kS™7âÅ¡?‹"44–ü?œ•þÊô—?ªgݜK©ï?ïx<Ü?"ű*vV?ZvÀµ?d˜+;ïž?›/úñ"?"²°}u?íîW9o'?ŠS‡yì?|ù2Zþg<?i^lœ
©?­{f§#?ŒÉìÖ·/-?í³þ}Õ2n?Ž%¸Q*?‰…~WôB?sˍ»Õé?®^¸Œêœ?‹gl¿¬54FGL J0253.5+3216?ï°yTª§3À7ÝÝãu…¾À:LŽ¶È¥À<VU°5½Q@°uÔ@9D$>û?»
Äv)?¢äž5ñ»?ç\V­‹¾æ@N;Qkƒ¿ïý‰-:Ë®?ïÿËA²Q÷¿åü&¡ÕRW¿âå`w9¿Ý-` Ô¡W¿äƒ«ñŠòAGNfsrq3FGL J0253.5+3216MG3 J025334+3217?ïúöŸØ!×?x«ÓÙrÿU?ÉgÑÀõ ?M»9Ãcå?@ÌS¥@†¦?tõ;V¯UÌ?ïÞÞ¾7؀?t
7™ì?B×2sl&?2&÷RàÍD?p•‡Iòý?s¤l	#t?ï'¹ÐH?€LÄü)¨?hA0½Ûjé?\ì@ž9hT?˜"Äʉš?}âãŸlD?ïñ3"^1r?Fü"wÚâ? ÊÚ½/>y?'±),Ð?[›ë÷1l?FŽ…¶4%4FGL J0253.9+5103¿í‹KßÁ5À¨—š¼À96Fñ'À;̯,¨Õ@Ä7B·`@‰Y_í¦a?±Q
¸Á?¯†ë8üv?úôš ¨4@×ÒÙ+Tí?înŽ¾tDu¿à7–oB­ú¿è"ÆÜ	¿âù'žªz'¿éI^]®[ó¿ïÖýÓ*	AGNfsrq3FGL J0253.8+5104TXS 0250+508?ïP¬ÅÂð?tÅG{?U"'ª	P?UºàŸ?Ù!?"''%']Q?Œ̳dÛj?íšy5^-Ã?µTû+?BW<{[Ö4?^Ju_E";?³‡ÜÚB?µ7¾uy?í×*Qölü?"'
L?ÊäZ^=˜?lÛöë>¢?®"þUMh'?'ÉŒã|Ä?ïm˙ªÓ?v´hÙì¶?g¡¸-ŒQ?TÒéB'€?Ž¤«Š=¨?t‡E¢îÍ4FGL J0255.8+0534?ëTìqíÀFÉ2µ^ñþÀ:½âïÙÀ<K4-@&ž'a™£@Ø8 þ?α^œÃo¬?¼µ‰9O,
?ñ£ø,Ìç¥@ªdSç‰?ҍyYˆ¿çCÞ¡¶sš¿áå­é¿¿à°
fóT¿èžP¸7ï¿è­ŸÀ¥!7AGNbll3FGL J0255.8+0532PMN J0255+0533?îóAð´"?"Þÿ}
î?Z"žcO?P­TÛÞ¿>?Ÿö¦=¿?"F¼™åÀ?ï@SæKþ?ŽmÝ
އ?M5*³©ÓÆ?VQ°-Þ²¹?—Ùàâá€?ÁRœ.?î1%`š¢ñ?'½1¹ÛXm?pmã'Ĥ?aÖdÏ¥H?ªßí"%xQ?'£ô‹z*Û?íÑÚ->æq?•×'¦è?hFû;ì …?Wïސ¸cŸ?°®ö¼)kv?™ˆ—U#4FGL J0256.3+0334¿ëÚ¾¿EªÀG}BÙÏÀ9÷íPÐÒìÀ<AåçP@Äþ¹®â×@"2A›«Ã?¶Œµ°{ˆ?'YÿáÞ=?ÝG!&Á4é@	$¼¥BÉ?ïû†ô{g¿â¤'ýuE¿ãÖÂ^ß´[¿ß3Žµâ¥¿Õú}¹©"¿ìÒ¯/-5AGNbll3FGL J0256.3+0335PKS B0253+033?ï³ñfFÛ?}±Vô ?C(7â¯p7?:±A¶Ô«?Ñ"ðGš?|±Ï§wË?ï¦ÇzW¦<?†Œ"¦·¯À?1#PË Tß?D˜F҉Å?…Åã¹nž?†# ´vÒ?îètNöýL?ˆ']xG¥?eH6ø?Tž2y÷^r? 'i¬¶?‡üªa:m?ï Ácfm?}…š–®LU?Y¬"ÅuV?IR:Ëi¯?šM';Üô?}yœZéˆ4FGL J0257.0+3358?ïè.ž	ôÀ6K<>t°À;ëÔÏÑÀ< ˆÛ¢@ Qg¢P¢Z?þÊTg`aj?ËY
Þ*m<?ÄGøý'LK?øz_\†é"?úW|5°'?ï'سiy¿îký^åé~?¾Ð_("ƒˆ¿àEéÞö!ÅL¥Ë¿çžÑ'ÙAGNbcuGB6 J0257+3357?ï'^™Æ'Ï?Šr4ŠÈ?JWc–\C?Dthµ9е?Âã\eæÈ?‰ÎhTJh©?î¢	­^­? ¶ºŽN?pÁKŠ}+?€ ÜXåE?£ÜﻸŁ?ž¸üêM$5?î
8ÍÃv?…OqøZ?sš4ñ2è?e˜†gÄëh?­|Ôýˆ?¤'™±b?êl7¦á©?¢1+ìJ\o?Žï—ì?œN?€e­|9?Ä`'èè—?¡÷pqž4FGL J0257.9-1215¿ã_N5(gÀLmîËûµÀ:6¯-•À<tÞë³Aá@ß?@1É@oœp
¯?¹Þ!
j¢?"h|ü*?ÕåFÁ/Š²@Õw®bS‡¿Úƍ«p¿å¯¿üò¿è…xDµ;·¿åP½Š'¿êšÏ>—"¿ïÿ€^	J¬AGNfsrq3FGL J0257.8-1216PMN J0257-1211?ïì>Ìs?]ËþÙN"?B'ЧÑt?7"³ºm·t?^¢ô\Ú?[23›`_?ïÒÖÎJOÐ?~mi&˜M—? ŽgÒ#?:¡f) ?v%œG–­?}†ÍêÝ@ž?ïN´Iδ?zŽ?O0¥-?g	\Ði?`˦£'gˆ?"FÕ±ä¯_?x#9ÇrX¬?ïèè=}F«?QÓ«
ꮄ?6þ½†Õí?)oå{=f?d7êÑޖT?PDë)y—¹4FGL J0258.1+2030¿Ö¾»^‡ÂÀ@ªé>›AÀ:k$-ܲÀ< p­E£@x¾'²!?ÿa­ê‰v6?Äðª7 ¨—?Ïuéüˆ|;@WÚè'®@	úâ"tt¿ïþsÙ°k?ïîQs	?À#^~æe¿á­:*ž9<¿æ¾J''?¿äûF'+½ôAGNbll3FGL J0258.0+2030MG3 J025805+2029?Šþ?"©Hè4e?hú	¨6™?hvØ ­zT?'ßšÖr/†?€ÎàLW&?ï+}t•M<?žvÏ	u¸«?`ðýfAж?~Y¥o7ˆ?˜r1ÀŽL?™§·ÌK­ë?ìû¬¥æuê?¡€¹Ud:?"87Ü
6?‰Œô­Z?³T—ÕN?›÷UïÃN?íkLT(>?'g/öT'¤?}`åü³Ï?n¶R€œT?±¦—="Œ¢?'Çu+Å4FGL J0259.3+5453¿é'J™x®àÀ¡!MW¢À:Œç='[À;́I@»²@ ¹zæ{¯@È>{?«¡ƒóÀ¿¦z¡÷Ùb?ç¥F`Œ‡¸?ñê2]ö*i?îpÿ¡á;Å¿ãçOš¿ç}îãx	ý¿ë‰ÝÏSÊ?кý Ë¿ßÎ59©AGNbcuGB6 J0259+5451?à™÷Ïm<?Ç;Á͜¿f?Ÿ²c¥Ái	?¤¥•b#Rw?ÜÒËÖ÷?DŽ×|ýª%?Înª˜5G?ÄJø;8f?}œ)œx¨?‹ƒÙÍÑt?è)SŸuK?Ä3$ô«÷?ãÇ
KÝÃ,?¯:¤? Ÿ7›n‡?ˆõdœÊÀx?Ö]ùÁQ×?­rÏœù{?ÑsÓ®<p?µ'Ðjuðò?‹·FcZ?¥å¬T?æיþUO?¶,h,
ˆ4FGL J0259.4+0308¿è*â-uó¼ÀGbŒ?>qÀ;zVÞ3'À<¸ÁDŽP@"uE?¥1}?÷è»ûÄ1?×›Á''?Áº	戶?ê&¿AžÛÎ@Œú–Àn¿ïÿ`Ï‰@?ïÚ ri¿ãÛJ¾ëԿَK½m´9¿×QmZ÷Gu¿Å^eYAGNbcu1RXS J025923.7+030736?ï±À²Žý¨?|ýwÉF?7[êˆÇ=?4ÀßÅ21?'Ôôî?{îLW¯?ïlÕ+;
?éÈŃ?CüpDD]X?W³îàiÀ?'Åw&u?NºXÍ?î dM?'5Žè»^u?j 0"
sû?SÂ)úH?®Sö¶ÿ?'Ü1nMZx?í€ãP‰…?žôÍ-czk?L~Tº¡J?LIKy"y?³¿èÒ>µÚ?Ÿ'×!O%4FGL J0259.4+0746?ë®é³žŽ²ÀE¨×¾˜V£À8¦ºò¯µeÀ;—ïrBÓ@qieŸA#@ùü£T-?¥½'&?¯Äà^ô"@	ž>^à`(@:ÍûXü?ëÄS­úпÞϸ$B`¿ã1¾Ý`™¿âgM"—¿åÈ×tÆ{z¿æª ¥gAGNfsrq3FGL J0259.5+0746PKS 0256+075?ïÈ2
¹¬3?pTçËðò?)¦*Sµ©Š?"F3wØø?{ÉPŒ9Ã?p-J¨ÒPz?ïÃÚèAå+?€oq­I¹?0§¿ä»ª?KW¨gkYV?}àÁ±?~ƒw<å8?îüz"Ú?‰Ýéä\o?qþÇ¢&Þ?d0ª‹A¹›?›ñ9Öºì?ˆQÜC­h?ïÜöq³~G?X,'#Éߧ?1cÊÐ	8?$t'-œŒ?pkÀé"Ûn?W…T©qÔç4FGL J0259.5+1924¿ïžÊü4¶ÀAÒܱF_À:y–°±
TÀ<#/V/@óôëû@õ
3¿?Âwÿk±?r§Î2s?°nD_÷7?ü€íÑ)Rà?ïl¤nò¿ã[QàG}î¿æ››œ©"¿âk
=²é¿ê4:WÎô¿Ýe5#xU&AGNfsrqTXS 0256+192?í#n8á%a?­ó¬»—?'+ÕvXÝÈ?{Åo>¢'?´ŸŠ+¹;?«´Ã~[õ?íù«''?ª¥‡^'[n?v²'ðÝ?ˆI½'Þ°?­	6t?§.DŽÏ(?ì­Š®?šÂùE÷½+?¼è™æ?ܓE­-?¶Ø'"Ë?—0ÒÈφ?és3'h? ±uë»ÉÖ?–ir¦Û—œ?}Àˆ›þ&?ÆõjVƒm? M'/ÇÇ4FGL J0259.5-1705?﬌…m¬ÀMcðí=…À;,>׬#àÀ<ªçcQ0@ Ò{ÿ)ì8?ùâwXüñX?Óô¸#G'Ë?ÙAŒ&êO•@¼[ed?þoKº">?ïôGe_M¿î½8À:î?Æk¼f£".¿Óx‹A'¡¿Þx'}sHL¿ïçB.x¹OAGNbcuNVSS J025933-170540?ï?@;ûEå?•¸È£k?U®8c#{?Q%ȼױÖ?–½úeÔ?•S¸ºZm¾?îÀõâh?¤£Ùö?r}q?ÿ?~
•qĀ—?¡¯Áiٍ?¢1ˆÑ³A×?ìÀäes? +Hàá?‹×Þª6Î?~©Ç²b8À?·—Æg‰?'_ÈdzÛ?é½Ø9ãà?¦2`Ú(?ƒõ%Úr´‡?w)¥1°?ÇÌFAqE;?¦T´wù4FGL J0301.0-1652?óºÀM-«KrÅÀ; g4À<€îßFL@xƒ/ö@A›@bƟ?Í@›üu[ø?§ê­ÞJ"¹?à÷¦ë@šÐ"Øi¹?—ŠØ>M¡?ï"=ý'·¿çU4_ƒV¿ÝRìÁ´À¼¿ç+=e¼{¿ïúª@/ðÞAGNbll3FGL J0301.4-1652PMN J0301-1652?ïéSãIR?[¼]™	"³?=ò‹l¢þÿ?9	™sßà?b"Nÿ?YXˆœ¼¿u?ïÔ«™¿t?}⍅¥êÂ?%Ūºº³"?>ìÊÙÞ¸?uG|ÝJp?|е¼Ÿ?îقÙ=íñ?‡»Ëd8?p&ÚŽ}´?g'rçù_? b÷,Q(?…ƒ
‹)Çò?ï°±¨W2Æ?k &âè<?No¦
®(Õ?AD Œâ&u?ì›‰Xl_?j.ì÷|þ4FGL J0301.2+2546?æè}0ÇÀ<ŽDR?gõÀ:ö} >ÏIÀ<dX£/D'@ÿÜ0B@ïêÄ.˜š?ÇnšgtÙF?§±U¢ô·"?àÊzw•bÓ?þ5&U)R4¿ç™ëcÉ?ê>zúr!†¿ß)ùc-Ì¿èiU./¾4¿âG)T ¿«-£SN(AGNbcuGB6 J0301+2546?îZ',
àa?¡-òÊÍéa?WéœTE'?QÏÆ邓?©ž@\±Õ? úÆ¯SS?ïöñ†!?•ÿˆÛ!7?W&ç¨Jv	?`¦Á°6?§?®³bj"‡?•V2q=ÇÖ?í"Àrԍ?"÷ÑOx0?Aî¡BO?qÙÐp!µÇ?±9¾§+»O?"ÚÙë¨?íҝ{¾?–¼é9Cˆ?'¦°Šm¦p?uû¦Sy|?µ£YÆmF?—-W»j4FGL J0301.4-3124¿ïë¬íšˆéÀN¸G¡A)À:ÉŠ ÒÀ<¼¨¨*V@áÚûä'@/S6L?Ã]:ƒ3¦¡?±ÒIäO Q?ì¼^'í0@QºÝ·¿Ò=?%¯½¿Ñ@{EE¯b¿èe¥@–É¿ÓüνgÔû¿éWÌÊæn¿éõF2ê8AGNbcuPKS 0259-316?îéͨ7Õ{?™X…5Ñ?k©í–ÏÊ¿?e:چéÓ?ŸQ
F+WJ?—áÙÓ)[Ý?ïuÔº,.?úï‰
ä?Myßµk?`V	¤ÛS?\"ë…äs?ÈvÅ?íÄ"Ëru?"œ¸ý¦?"9gCÌ1?wí+Áç9¾?®»Ï¹wå£?Û³£Í7?îó8Ùv¥Ã?'fvÀQ^?vT¡tì½?dß3ז[À?œ¼Î•?€‹íí"™44FGL J0301.6-7155?á÷IF+C·ÀDã[ÕìlÀ:"ïÙAOVÀ<Š³Ï¥Å!@'ñÒjÆr@óÕ4z[?¸a=݆.?°¸9þå‰î?ô+¸e6»~@Ÿ®†¨?Ðt=$à¿ã4ÿ@'lT¿åf‰l$ìI¿èrNf•`O¿ì°a¬m\¿ïðȊGìÿAGNfsrq3FGL J0301.8-7157PKS 0301-721?ï«
Ͻ¥?~±³}h|?U	åçÕð ?MÈ+8)?'›OS›þ?|ð	nºö?ï©t¿؏?‡¦ób gf?6—¹±'c÷?M0éäšÃá?"îo=I2?†Š àVÊ?ïQXX*VÃ?{¦¨«ã?kªŒñ‰?Z*HŠSØ?'rÿ¸ƒ‰^?x°"¹ÏùZ?ïǔÄkf?bõLcÔ@'?`Na;@"?N¯7M¨?tm *Kå?`†ZǧÜ4FGL J0301.9-2731?¿%'ƒŽÀNŠó¡LìBÀ:©·¢åsÀ<°XaÀå8@-^g¿Ví@ˆÐâ2?Å.ä —?»œ©'ý?ö8›P˜Ÿ@3êrúôR?ï¬W¿ãž"Ô]ºÆ¿ãÓÂT£ÆC¿áÝŸ¤u–¿ê2ËŸ¿ïÿ3Qf$!AGNbcu3FGL J0301.8-2721NVSS J030158-272754?ït'Y,†?¤òc³æF?]ù0½|ú}?º?dxÊ?ƒ.ß? ¡3ßvïw?7Âà?‰›·C*\)?@bÉsŸHç?P\–Æÿ«þ?‡ÖE"•SU?ˆ‡ #8	%?îêñõ±?"cQ
Í\?pZ"›¹i?i],·àÒe?ž‹:º[ý?'
™¼+oˆ?ïsC±žë¢?påQ¤¢ß7?fHå0Ú?R5?¼ÚBö?^åK=?nÝöL¸J4FGL J0303.2+3149¿åç[=ŠÇfÀ76˧2ßPÀ:hµ}$îÍÀ<@¾(Å@tÙrÍ|ö@i=Š¥
?Å-h±Å4?Än³&ˆì?ÿ»iGÂ6q?ÿÿ—ðw ô?爆ìî«D¿âÁ²‡§(οã%Ɉt®(¿æj}ík¨Æ¿êHuà+ú/¿ïÿùëñAGNbcu3FGL J0303.0+3150B2 0259+31?êâ/öŠC?´H½§y~â?¡LâŸ1'í?–¡Ñ.V®¥?À$~&s?²Á}Oÿ»{?ì¢G0®Ôç?°	¸Z?"Ì–.Šå?"b{0aõ?µúÆTý¶?¬0ã)¿Ò?ì2®Í¤? vð¯ƒ?š°j¾Ö"?ˆr˜úߑ_?¸³ƒºÔZ?š]ʸAo?掜VËåV?¡ü6d?°OI'´Ý?'i4É¥"?͝ê#4? í0"SFü4FGL J0303.3-7913?í…U§ÞÀAý´þyîÀ:F‹yEf<À<c@þÍÐÙ@rË7@‡¤¤—?½ù
†? Ç†>?ã	Õ×7‰Ú@
€«Œ
e¿Ñÿø^¿ä"\0ýN¿égþìډ¿Ù@ÛýÂ8¿ë¾Ïÿ1N¿ïÿLkAGNfsrq3FGL J0302.5-7915PMN J0303-7914?ïä°"m?bÀ
‡X?Es†ÚvŠ.?8›W"—ß?fŽmµ`ñ¶?`þ#S×®?ﳖ?Df"?ƒPE:R±?2,áùFH?Eë‹~íNä?'‰g֐á?'ï†{×s?ïN"fšs?{¼æq ê!?krµTb"?eÛªcràã?'¿L'%T?wÇ]¿­µo?ï¼ñô}i£?cô,™X–?Yۏ"Ñغ?G¶*6W'|?{!ÜV¸X?a3±Ÿ‰û'4FGL J0303.3+0555¿â¤æ¼ž=ÀF-û¹À;Tšù*4À<‹ºˆ&ª@"¡ûï»?øÿø¨ó©°?ÖwºKÀÉ?µÎî:/Ѫ?âºcslß&@bü]^*?ìÈK~ºE¿ïÿòß0&¹?ïþ'¨'Y¿ä«­Bm㳿¾Ã!¨FZ­?‰R Ð‰^¨AGNbllGB6 J0303+0554?ÚãÎ$?Ä'Ÿh­¥?@î´3'?8ôŸMŸ¹V?£Ã*òOy?œ!§†x?ïlÏ4e?žŠ5Vǒ?ZrâȐ>?oÕóXj Ð?œ‹O™™:E?›À‹Ø]-?í_ÑÏÆL?–£âWQ?q‹±ìö_B?b硾{?³è¶h:g°?–n[<²?ê$N7QõR?°ñÞSrÍÖ?Dq‡/°ÿ?Hl*@4À}?ÇZU›‰?°ó'ðÁ¬Ý4FGL J0303.4-2407?áOòÉ-'xÀNŠ›ÏÔ¿À7¤¿Ä¦ŽÀ;'­¯Ñƒ@g½ml
?ý"«þöë"?•p³W–ûì? w›ºR™@<ï>çœ\@š'ျ¿¿u š"¿×ö‹ÂÁ[*¿ß
X^©¿Üª½"µ·‡¿à·4µs¿Ýìðƒ¶-yAGNBLL3FGL J0303.4-2407PKS 0301-243?ïÅæϲ{†?vǨ
[p3?µ[d®+—?ã6»@À?|'¹/"?v«¦TSK?ïԌafƒ=?|Çú&${Y?-í¢ãô"?F`°'§¿Ç?tÊb5žÁ?{·N˜²Ãº?îOf[ÚC#?˜½¥)?{ÄC%vi?xý›ÅÅp?§'ݸ_?–¥âùÔfê?ïîkÞäå?Sìk~6ó? da¯	À>ûý¡»ç{?aM Q"]"?SЭf§h{4FGL J0303.4-5232¿ã3#¸ØqÀKVx|é_«À:NÇw"vMÀ<mÏt@3ÏDvQ–@Ð"<jêZ?ÄE¡Iç*?ËЗ;ÊÜ@c±€@,@@rwÅç«¿â\^¿âⴕžbV¿ëf¿§ C¿é©Ì·ÔD¿ïþÒ8F˜k¿ïð®SeâAGNbcuAT20G J030328-523433?ïði§Z­ª?ao_Õä'?IkH¿‰C?Sm»½‹Ç?Rwêàu?VL#:H?ï'@Þ¸=?ŽöäwÁŸ?DáýÛ!ˆ-?WºƒÅyz?Š!¸ªŸ×î?y÷øÌP?îÁÔZ±b"?‹:UÙ?UžŒµ|?tõ²2/a³?Ÿ¥cxý´?…Ïz*»?ïÔtÉâþx?`$™v'w±?UŽäW֑?E+7¼Ä¡D?pbÕjÎU?[ì)`¬"4FGL J0303.6+4716?ìk-†SŸÀ#µx_.QÀ8rÆ	d,ÐÀ;˜äXڌ©@ˆƒÇ =@Ǧ†è½?¢§û\,PÁ?´Qç¾Àš@H<¯³·@Ԓ¾Þø?ޛà»íŸ¿ÜŸF¡úç¿âŸA¤:¿ã=OK—®¿æЎÞT´¿àíñ_©2êAGNbll3FGL J0303.6+47164C +47.08?í,.'Ø9?²íƚã[º?c]»üy}?bçðîí?¶«°«q¶?²£¦ÕÍ?î0A´"Ö?²­ô¸ìcù?bÞdAIó?z ‡Ê5ôU?«Î°z
í?²5oõyä?î}
ÿd?"o=×JP•?ƒC†®¥¼¬?€GÞ/a¯-?£^n[dê•?h'w?îý'Ñ?Â~R6¬S?{Í2¡{Ë?eÊØiL?™j¯¥GH?€8_Gÿ,ë4FGL J0303.6-6211¿é—«OÏvÀHYå\ËOÀ9Q³ø^KÀ<êg¹M@¨3vë@Ùb<5:?®É)¥?¸S´²ú"¯@c¤%
×@‰ˆ)"´¿ÞpGÛá½ ¿à6¹?|AÅ¿æªiËuµ¿äZTª|?ì¿ë(ÔɎտïþ²í'¶AGNfsrq3FGL J0303.7-6211PKS 0302-623?ïÒPÇ¥;Y?pÙ%·‹ôÁ?Dr!Ú耠?;‹ŽÓnàã?tIWòC¥?pîÕwwl?ï¸áánÖ?ƒ1 ±fEG?2*š£?Fù¬áפç?6þoy¸?'ŽÐjwSÈ?ï֖±³T?ƒª
€fs?uŒÿÓŽÜ ?h'!ÄÉק?˜Áí4åÞa?œÓÙP?ï֛x†>?_ŽTè?@¡ßt3?2"Þ,)<?rž"àÎZž?]~	†é"X4FGL J0304.4-2833¿ët¨úýžÀNU<æÀ"À:øÕ!/$±À<˜5¤&»V@! pe˜¶?óV¡—"Ü›?ÙÃp,¸Å¯?ß(Ì|ðÁt@j¸A$@eK#É3?ï÷D9ë´?ï¢.(1wq¿å°'b"s?Ë´¯¼пݳÿ¡`bk¿çûûŽ7£AGNbll3FGL J0304.3-2836RBS 0385?ï?ÿò$w:?'G©DP"#?}<c'»'?wHÿc9ðm?°ü"Œ©ë?Œòõ½'=?ï¨Iè6?¢ª°é*¤?râJDzan?•©~ïÃÓ¿?™rdÖ`Ï?š>±Ë=<?ìŸ%P½ù?†5ƒO?'‡¸ˆ…R6?'ý\§fÅ?¶e³X»§?™ä‰t¯Æ.?ëè€á£?ªz‰–Ñéš?3ô©ÌB?`^šñe?¿Åc¹W?ª_g<V…4FGL J0304.5+3349?À¦—®ÝÎ}À5\ÂÅâÍÀÀ:ˆÝÇÆӏÀ<ڀ¶–@ò1Xèy|@æΆ
pœ?Õ
å=‡?؞œã¦3@_¶™" ä@%#ûݱ¿ìºÁ5¿Õ?ëAµ!_v2¿ê»à¡¿éáìžú+«¿è²2·ã0¼¿ïéXü˜AGNbcu4C +33.06?ï»i<çün?~Ÿí²5?y#?ʛ³G?yÕ°Bã¨?bPC'Ì*/?bûGï´ÿ?í»ò@wwµ?±Ø»i¬îp?"r¡*3öë?¢o‡Å»¾?ª‹cn‰*?¨È¥Ñ|/?ëg²
kÏ?¢Ršá;Â?£g¯:§ô¾?''u{&b#?¹`êÒ@§-?àOCi¤S?ëåÔ8)†?¢ú[Ù\M?¥£^¦ºnm?"ªÌ"T¾?¶R
á| ?¤¬Nã~ÊÑ4FGL J0304.5+6821¿î!-ræË@!.Ÿê$ÌÀ8Í~¼ž`À;SàGÓÔ@^^ߎš@[\|ؘ³?°­xH¼?ËK­h¿@U§L	ÃÎ@H®ÅzÉ¿Åçû;õún¿â½:ZMS¿èXžâ¿éÄÜޒÇî¿ëyóa2¹¿ïþú¡Ç:'AGNbcu3FGL J0304.9+6817TXS 0259+681?ív´ô]»\?¬Ãh‰÷ÙË?¥›Ò‰×'O?¤Ü1s+2?¢øÞ0L¸ø?ž'"q‹?âv'¢¹%?Ñ
§áÈÂ?Ë#Ü$
Lç?ÊsõÏct?ËÕÑj΃?ÆÃÅ(鳿?è:Ÿöº}?±¥ÌA‡åå?Àµ–2c?ª´ðP|=?¼¿Ô>­f?¢ÿù¨)'?Ýúm¶ŸŸ?°!¦‰ˆr?Ç¿®G‰¼9?¬(Å!"I?Ö%»%œE?±èç㴕`4FGL J0304.5-0054¿ïßAº=0ÁÀHXǟfb5À:â,[ØÀ<žBuÆ@Ì0ÐWpÕ@X϶¤l?Â.ú(ûvÙ?€åƒõ9õ¼?ÀqU­±~"@³>†MŒ¿ïû–ÿ‹eú?ït¦Àž–.¿à(é}Ý{q¿å
*Ž:Á¿Ü"±þ?`"¿Ê¦2™°?ÎAGNbllRX J0304.5-0054?ïÍS
x?ugñ².P?<rD™Hcâ?;"yËU°?w®WŒæ>t?týLn'3?ï©Ùû.?"ç§ü¬]'?1	@þ•}?C}²2j?…3ÿy?Ì´?"@W‹ã?î-Á\¤?2B Ljå?w8€p¦ÇŽ?h{"¬è	w?ª<Þ¬ åÛ?×˜VDÔ?ïKRcžó?zHTª‹?R±õéJs9?F©ü"'×ú?•t–T÷zˆ?z$t¤£Þ4FGL J0304.9-0606¿ï¯K½BÁÀIû5ü;OaÀ:´BˆCÀ<|vOèu @Þä^9@æCåÍ?ÊÅ4'$E?¬nÊcª?à52F¤)@@â)é•ö¿âÄâˆô'¿ÝG­¾"¥¿¿â$ýh %¿äL<ÿÂ«¿ã_iG¿ïÿþó…õAGNbll1FGL J0305.0-0601PMN J0304-0608?￵žNK>?z·ó…þ¨b??­ó氆?6Ùò‹Or?~*`¹›õ˜?z2ÀîH¼_?ïŠ=¬ Õ?‰š-®¡?;+Ö	'˜?N'eÞïœ?Œ—ev'~S?ˆ²ð¥÷ ?î±×¾'ûù?ˆéŸBga>?q!Å ¾°?b(åÄù¦?¢¾Kuœ( ?‡3µ&UÉ?ïoqN]ÄÓ?tŒƒáEœð?D7ÃH%¤8?3§p†Ô¢?'p8€?tO2N+'l4FGL J0305.1-1608?èoŒ·«IèÀL•!Ý Y§À:€'_ét£À<k7…¨K@!	‰Í?û€N¤¨ÁU?ªÄw=Ï?®. |wJ?îÚ³	­'ì@
þ"™Or?ïÆÛl6Š¿çµÞÿT^|¿×ÐPåË¡T¿à"H÷À–¿».ù<ÂS!¿à.ŽˆÄ_AGNbll3FGL J0305.2-1607PKS 0302-16?ïÈn²ˆ¢"?r$Œ¿º?3짞œY¸?*¥œ'Ÿ'?z‰ÜAÄðý?qÒ¸6»ÅÖ?ïÁÐ9¯Q?'n¦	÷¢?*è0˜¥O?@m=5g×?~ŸV^c*å?ÑCÐù2Ñ?î_¯{ñ¨x?"¤k"¤?a=YÍáI÷?\æžÞ²[?¨ñ2¤cð?"Ö¹8-?ï*Ró?mëY̊$?8ý½Öõ?2íÈ@YÙ?šQʦ™Þ¥?bîÝCAŸ4FGL J0307.4+4915?ïúZ"ÀGc€X€À9
¾.¤XÀ;ªQ­q½²@µ$h?ÿ	GŒ†‹ ?­Nçï'õ?¸ Š6Nœ@©ÊAR@ãTpšœÏ¿ánoês¦Á¿ÝÃT~–¿Ù3$º¼)¿âÎg öo³¿ß6#¨{µ¿åû¦Ôë?AGNbll3FGL J0307.3+4916GB6 J0307+4915?ëa-ØÀ&?¶AxŒA ?s½CÐv?qnÅyRDî?ÁÝaØD8ã?µ'Fíò3?èß(ɉ:?ĽË>q±>?~)…XЫ?¨÷I«Ž?˒^[?ÄU…Çpþž?éëÊ`1Œð?«EÙ^½No?›<Êü…Þ?‰ÖlxÒIv?Äé=©)f?¨hâPU•U?êÐ|Ä+ú¬?¡Y0:w¹¾?"w‹C‡2Í?|´põXÞ¯?ÂO†ß.ó? žˆ£žêE4FGL J0307.8-0419¿Ç6€
¸{îÀI%ŽÉ[ÿÀ;`ØÞ¨—À<°yixiž@ÆðŒÅuÀ@ڒ_ét£?Î'
)¤"?xÔ â«^Ó?¨D<ߞ$ˆ@åGÂâ=?ì©ðÿ±üg?îâBµ‡5ê¿Ý‹@»\¿Õp^aàÜ¿é'Àoz¿´ŸEÀ~ŠÊAGNbcuLEDA 095522?ï¶aq¥h¡?w§°5!Cü?U+f'‹?Q÷4Å;?"mŒÈY?v…m c??ï–Â?‡Ä·v-?;¤Úõ¾¤?MQ_yeFÔ?‰v¹§Ðó?†Áýï&áŠ?íõšT@n?4E]š&?|€·"[~?r´/òbŒØ?­GZi³?ŒZ.»Æí?ïFmÈë\?'±=ȒÄ?cZK{
‹?W4½­›M?"Ç—C*?~÷&îʶ4FGL J0308.1-2852¿Ðú	Ä­w%ÀMðX>…vÍÀ;`Á¥À<ĦÚ'Q@À$¢ö@_ƒôç?É秄ô¤?´ßª_‡?èC ´@ZÖ¼å¤?ïãq¿_üÀ¿ã0
¿0W¿Øò@#Ü~¿æH¿AHõ'¿Ö
HÞI"¿ïÿ·Û¤%AGNbcu3FGL J0308.4-28522MASS J03081686-2851054?eY"ß?…pÚg½£¦?H[õ[¹ØË?@ˆqÏÙ[?'Sß*¦?"øgðåãø?ï"AL??‰ùE'w>??ôâðÌSÛ?SÚÌ6ÌY?‰ðص?ˆïb\‹ß?íùéíëÈ?'ðÞ\lÒ?tE×!,F?g‰‹e2ß?­Ø¦IÛ±?'
=E?hž?ïDÒ
‹«ƒ?{',€_Ñ?I·g/áB??ãq³Ê¢|?– óQ"?{5Zef4FGL J0308.4+0407?Þ[í!èiÀF@ûüe@ÌÀ9r×;»—ñÀ<K]Ìcñ@7žÐP?þ"°hè÷¦?²rÐWîï?³»ÀNÓç@Ôþ¢1î@
(Kù}°¿ïkL"=?ïôµ^œ£¿à}Ôvå9«¿ÛÊ÷_tp¿ã¸ÅÿS1Ö¿ÝI‡Þ[?—AGNrdg3FGL J0308.6+0408NGC 1218?ïןe®óˆ?­J"ϗá?;KqTW¯?pü|ì¸'?r{– öÙ?«*¿`Ûê½?ï¬à‰Ô%?ƒ‰â'©^>?=r%Æ×y?R¾lãÐw4?ƒÜLb ?'Uu ƒ±?ïÙ³^‰ô?€oDú3?iÄL7pI	?]J,Á§?™Œ@
@¸G?~—4¤L'›?ïx¾œpM?rÈ|~`­?cå=Š?QÆ?
×Â?3×	¢J?q&/\…ú4FGL J0309.0+1029?ìwôЙWwÀCÛ×Ûô‡ýÀ8ÜG©â¼ùÀ;¬éïóB'@e'æèW@Îy$¯ò?©çØýî¾ö?½Zç,IŠ
@´'\e[¤@ÕH©0տ؏ØÛMîö¿ÜUÝað_ú¿äEÂÖ[¿ç(àwúc¿çH©©µ¿æE»ãAGNfsrq3FGL J0309.0+1029PKS 0306+102?ïˬyey?q½Î+[ŸF?:c¶MX>Ö?På&
¦Ë}?xƒ‡è¤?C?pˆJ\<½r?ïÇǂ@‡×?|?á,‰‹?1nlö²:?FM¤ý\ö?{XPòå?{)NU¶ë?îӚ?ŠìT´é?wMK…³?q=øÔçNX?œiªÒ«Y?‡§ªØJÍ?ïï.$'6Þ?K0§œÕy?	$–~w?mb.@ç?`	'Œ¤mŒ?JOA¥94FGL J0309.4-4000?Û£$åÈÐÀM`_ö"FÀ;[­÷õoƒÀ<ÛÑ_ÄÖ@ ¤{jÚin?ûæ ÆI%
?ËÁ>â=ø?¼(ÝÄÁ»w?óܨ##ñ@ïkY?aj¿ï€x–Ó?ïý Ê]¿ÛD!=<v¿Øtâ*,#t¿åjÛuÜûï?³¦G":AGNbcuPKS 0307-402?ïÖYMx>Ž?fo%èÒ?5Ã'ô[h ?.?dMµL?sw&ě&?e–j]Èyâ?}5bÕ?ˆrva	7?;ݯB¤g?P8ê€òP?ˆ8ó5½5½?‡šÆÂø@Ã?îh— ?ˆ¶õ/y™?nc€¯mÈ?XK€æ'à?§˜žƒˆ.?‡Ž÷zÝp?ï‡uÁ›Z?€¶I˜è8?a86£C?T
ÓÁîÝE?™è!`H?€"È	šþ¿4FGL J0309.7-0745?îm&|ŸÀIükßL+RÀ:`ۋ¬q
À<b//˜t@Çñ²µI?ýï¥Å!á?ċ–€_Œ?·›ùñ9!?ñÀ£"î^î@Oá>Ê?îÂWþė¿ãW²8ÌÐ(¿ßT|Yó¿Ç˜iwÿk¿ë˜š`höd¿ U8»]dAGNbll3FGL J0309.5-0749NVSS J030943-074427?ïЖúñz?ŸÓ7Hf?d!ŸWÔÓ&?[j6Gò'g?šá¹5§6@?Ÿš"
j?ï`×\H?"T'ñöӚ?Qróœ®ç?eìј^??'æ5íº«ë?'ÕÁ"û<?ìâ×6Z;[?›¹ÔÒᚍ?"PÑ*ï*E?‹q*ûÀŸ?³ÕrZ"?"qã´x?î*z([ӕ?Œ;N̆?|>‹µÄ?ktG%Æ?©Ðœ·Oï?Š[.·!24FGL J0309.9-6058¿³ÞaÀ¿lJÀHxj¹¦À8c9‰Ž‰›À;á"0ÉÌg@ýØ@N°œë]²?ŸŠz¨ùÅ?¹+
÷fÿ@‡¹E @¥K#É3¿¬Õ²_ÊQ.¿ãP;å‰\¿ç1tØÂú¿çÖÆz£¿é¹…\˲ñ¿ïïÉQIÉAGNfsrq3FGL J0309.9-6057PKS 0308-611?ï¯'–N¶F?z`'Ñà?dóRR´)?]ß ÖÜàs?}ò‹¯JÈÝ?vÐdŠWR;?ï¦dû:áó?ˆÿ[ÀÅ
?E#­C¬¡Ê?hnQáuq÷?…†]¹\?‡œ3µÖV°?ï@§ªo¥?ƒÃP§"@?wwc¡o{Ä?u—oñö»?'
1×,…?~léAøŸÝ?ïðó—!?MÇW–¹Ÿ?7Jë]g_?.R,´.?XU?	eÑ?JœŒw|›[4FGL J0310.6-5017?îæÜ@ïD­ÀKmÖ¾¾QÀ:*Vˆ¢ÑQÀ<a€OE¸q@ yޓô"?üs$ºÊl?·•`ÏΉæ?©A|÷øI¨?òª—ƒ>äA@%"z£Š3¿à=¢wŽ­?î½:¾AÓuNÌí¨¿â©?ÿÊP¿¬yšÜËٙ¿çÝúºpªAGNbll3FGL J0310.4-50151RXS J031036.0-501615?ïõÖô´¡Ð?K˜"Mkô–?&Uqïô?#'[·"?Q‡hdØÂX?I	pCËì?ïÕӌ?I?{8ނ6%O? Žu•ʁ?@Ì\yab?t7¼ð?zëZ4²À?îбºBc?Œ£;ô·ð?i˜dYœl?i'WžêGú?¡[lŽ?î?ŠÏs#åÔÆ?ニÏÞô?hÎí{wnÿ?9s!ˆ¶î§?1µ"FõC?%e÷úŠl?hkþª0I4FGL J0310.8-1041¿¿ LєݝÀJ¬7'MLºÀ:þˆ†KÞüÀ<‡]°µ?@ 8ä¥Üs?ÿë¯æâøˆ?Ç-fe§?ž¯×žŒón?؆|¥@¶…8?í¤.}ÁÌ¿¿é2þ'W¿ÅÞo¡ùd…¿è¯Þ|¸¿ÒÔó"õH¿Â.åE¿|ØAGNbcuPMN J0310-1037?îZ­sŒ?¢`[¶:Ì&?QÀu¨Å¦à?C¶O73¶?®üQ¢™í?¢Am¯"‰â?ïumî³ì?\'þۚ?GVÃÏtwÇ?Z#!º	?—ŒÛ÷?6EC?í»æçNê5?"x±ÝÚNS?rB<6?fÕG‰¸Oq?°ÿÏÁdêü?'|–*ëG?^¹e7?‹b/¨kå?GÄaõµ–?@é©Þ¬ }?§¹úáÕ¥?‹pT8hÒm4FGL J0310.9-3458¿åþVèoÀM¤N¤¨ÁUÀ;cârPÀ<æTe²â@@D[GNs+?ýÆ,Ÿ›;Z?Õ:ý Ë?ÀáŸlÂK?é9¯ž¾œˆ?ù-‰Ó¨ß?ïüà[
‡¿â˜¹Z)A¿â‹Y?aiÒ¿Òɧ~^«¿ëÒ/]•?Ջ÷-âAGNbcuGALEXASC J031057.27-350033.4?îþ¨ËÞóÜ?šn´w©ß?RÆÅéPÄ?Q^+Ñ?žþz%Œ'ç?™°ÝäC"\?ï-öÎx7Â?—¥LsÔ?]D
{: Ù?jb,)5œ'?˜låYE]©?•×ŒåTŽå?í¢xn†õë?"Ä?ƒDüqN?y¶¨dú?°ƒœý¨ "?'3nÉè(ó?í›Nc¦À?–1I"·>ô?rŒŸì?dÂ&ˆ¯Ag?²\š0?•ðÉ´Ãí³4FGL J0310.9+3815?ïÂÿ•»­ZÀ0ëã}é9ëÀ:
ZÊPñŠÀ<:"^žñÈ@0z·\Ç@qg#$È6?¿íQ҅že?¹Ç}W™™ï?øÒÅjüZ@äl$ko:?ïà«ÁºJ¿ç4éKˆ"¿ã â-‡!È¿á³/'N¤S¿ío
D& ~¿ï×ó;Ì^éAGNfsrq3FGL J0310.8+3814B3 0307+380?îû…欖{?—0'¸kr"?hò¨
÷8?bƒôPØ»?pî(®Iž?–›IÖe?ï\҂ðò~?"†Ø­c¾?Zy3"¶3Å?iäi¸D?'¾h¦M!?"!ƒöI*?î#Ç %­ö?•-«"?Œa(•Ýü€?…;©=
?¦«;Ø-¡z?ÚDVF»?î(ca¸s?‰ëä'<?'̈Z?y±jþ`Ù?¥§5Á˺?ƒF%s6՛4FGL J0311.2+6856¿ïË1½Dø
@"͒·þ¯À:¿ޱџÀ<2$fÖ@ ¯ø
é(?û‰Uê`o?ÒEÇ_zŽç?ѝbœ,p÷?û-%g˜•Ž@ æõ—ò%¿ÉÞºu‡@§?ë­ÃAޜ®¿âò¡r«ï¿Ùˆ›dÊÚÚ¿æ$ü=s¿Þ"˜±<MŽAGNbcuNVSS J031111+685610?ásñ"UY²?ÃhxÙáö?€èDéþ?zúV1Åm?ܐڶöž?Ãq$ŽiÅ%?çÃdYJšñ?Ç>ô'™ïØ?›'ú|
V?‹ÓõðòF-?Ïصk-Óc?ÆՃ(³…?èkªq.*?ªˆÕš9ê°?¿ôìy"­?‡h]=ۛ?ʙW¸¿?§_K(?évG
á?¢¶M[º/ô?‹Eè‹Úù?z
ogöWq?ÉýÈ[ÂÌ?¢|üß]¶4FGL J0311.5-4402¿×{ŒSòÊÀLž¡3ßÀ;e'Ýãu†À<ãñx7@YvT3ˆ@pµ'-lJ?Âϼ<0Þ¿©in"?åkÛ@#œ@,¶ùPäI?ëËw͖÷(?í+¡~•\H¿ãÝløPß¿ïÿ ÿ¿h`?ïý''N#z¿à¶Y"±ðAGNbcuGALEXASC J031103.24-440227.8?ï騃RéÇ?düRxÖãy?5¯KH<\?4))­W-?c¡"D­q?cÏRú¥é¦?ï£ar¾?"Nu_6?Iÿ~?tI)?iÀÑwzh?…‡Ã?‡$?¿ï9ö¯ç?퐇|€²Ñ?—ÑpÂ?€^†
`=»?{Ðë5/™N?±oóZNaÑ?•£N¥vÇr?ïÜyÏ\S?iÚ Œ¨\?<w¢ÊÜî?tp·ðAj?q°Ñ9Æ«B?i®eHØ´4FGL J0311.6+4134¿õ.&LúÀ,ô{gkÀ;z/—@À< !úü‹@!mˆô…Î?úO}¶åû?ÙFf@Ѭ[?Õ,ÅÛÁÝ0?ùoz^Ù@g"#ìÞ¿Ñ5®ÃLpq¿çæf0¶1¿ìNÚX¦ŠC?º#Rë__¿èe;ÞÓ_Ž¿µ 8š%Z­AGNbcuB3 0308+413?nM? âÞ.t?bD"Em?bNb6¢G"?¤òLXöÝz?ŸJØcY¹J?íšEpRD ?»á:"	`d?k8f¤TE?~™íæLT8?²THIXc?»†'-¡º?í,ÿ¥™3Ï?›0 f.†?ƒ\~»Zâ?uԎ™˜S+?´,Ã^ö*?™C7ßBÄC?ìAÐÃ}D&?¥6ŸËÄ®É?j‹™''í?ié€l¨9?½Î™?¥BEw˜Ù4FGL J0312.4-3221?הª˜*¿ØÀM‹ºÜ	€²À;ylÛM™À<÷#a	/@Þóú?üã¥Áƍ?ÛæŸê$Ì?Ñä"''?úNãx	üÙ@ía½ª?ï±ÊÛ[¿Ñü×V"ŠŒ¿å¡@Aº¿Ì!8	ã¿è)Âbæ¿ðAGNbcuNVSS J031234-322315?ïÆB22ÿ±?rŽË(.—?Q;ß±8+÷?IކO·?xîú2,?p»«õóYð?ïq¯ºì¯?¯ËF[½­?Iù6…¶Ì»?V=³A<»^?úS"t³ ?
N²e\]?íњRçWZ?"/•ˆÝ<?†€hŒö&§?w·«jáo?­F@®M¬?lã£F^?îôW;ÛäH?…ÅFº¨ËŠ?bTÝÇáËE?^š•$SÎ4?Ÿ*|ˇ=?"ø8!¯a4FGL J0312.5-2221?Ð?	)8LfÀLÛƒjƒ,À:8†-¬
µÀ<bãv\}¯@ N™@-m?ú®4Ʊ)Ù?Àtv‰õÛ?ÅF×)òíž@I¢ÿsé@Üwý½…‡?ïÿì´É È¿Ýq ~¥¢f¿°¸'Ï&ï-¿×⛠}.¿ÜXJy¡¿ìy&\‹RAGNbll3FGL J0312.7-2222NVSS J031235-222118?ïWàtjx9?‹'x5ŸƒI?gÛí·tRœ?f± è÷?'s»Ânh?‰!€fMS?ïc¦—o®&?"/˜ùx›?U7º³z?fíb'î\?'7´@n?''¸(—a?íC†œWßt?™Í•"[?"ñƒَú?wRöÚzñj?³Eš¹e҂?–çaؘö?í{Té<-?'V['s–?vÜÌþ)Øë?bÎÉÂC3!?²¹PˆÓ
?«±Èý˜¢4FGL J0312.8+0134¿ët³¥Ö¶'ÀF½ke©¨À9ƺNEqÀ<(ó"Çz}@‹‹«sÄ@-òˆH?ºùµkŒ&?¶U¶ë¹÷Þ?ù˚¥—Õ@»I)"£æ?ï͐â:ó¿Ñ!DÚ$¤¿åMú>ŸøÙ¿ããe€À¿äéëÁ"š¿ðAGNfsrq3FGL J0312.7+0133PKS 0310+013?ïæ¶×Q1?‡¹OðPœ'?3æ)ߙ|?F¯ë1*E}?g‰crÚ ?†Y6~ô?ï»éÎ\ª?'ˆ7†Z1[?/íÃèŒç?PäÙ¹L?€†À
3P?Ÿ×U·[?îé¾{¬X•?‡ª»~?uEWðôÞ2?j'ái?vڎ7µÝ?"ÝàÍu?ï¨ÄŽ;3?jÕaøÙÊF?O1³–?>‰…mÓÃ?ƒÞVRg?i¸A
/Œª4FGL J0312.9+3614¿¥'Ù•†Z:À2i¶°_¯À:ieõ'_À<?
 ë2@ žôÄ7§â?ýYÞ7X\?¸Ã…¦G§ß?«I­âÀ˜Ñ?óÚE[Sã­@±(Íÿ|Í¿ïýgß?ïãϝ·‹r¿ÈqMàˆ–g¿Û±dÜ£"¿äeÜÓ«
¿ÃÏéŒÌAGNbll3FGL J0312.7+3613V Zw 326?﮿uíµ??vžÞöÔçã?PÂÕ	Z5Q?D¬Ç¥|?'7Çãgi}?up˜­«úá?ï~ke)0P?Ď
×ö?OÐ Ïýg?cCW"$ê?Žh$¨ÂlP?Žx@Dä?í]š'Äû?–¦¡-'¾?'ض57'o?u±ŸZ?²¸û1>ª?"GàIl?í›Kt¿?ÎÛ\0Ü?‰¦¢2hJ­?r=*Ž1äÑ?¯á§<$'d?‹ŠÛBmr4FGL J0312.9+4119?՝qEùšœÀ,7A¿½ð'À:7"¶
m§À;
ñû@§Ï"þ)f@+¹!]¹?»O'ÿƒð¿¿W4ð!»'@f"f\Uk@	¼óíx¿ØÔDRÈû¿Ëcòl¿Áj¢
Vp$¿é~0O‹Y¿ÅV1ûOÂ
¿ðAGNrdgB3 0309+411B?ï
A›6¿?­»Ÿ3³=?kz¸à[€X?r;x˜Ø ?›Hu}­l?¬6BXzÂ?îçÀÔ³ß ?¬ÖÞi"‹œ?n[éï€R?‹é´1yd?Ÿ<h+"›?©·JUI?ç±åãOpø?®á╳¾õ?§þÄÑo%?šÔYšìc?Ë8ãàX?ªåÂ:º¶?æz±ËÇ?¾;£¥°xÄ?aBÎ&iUd?eè='`+
?Ó²†JO•É?¾)ýл!4FGL J0313.0+0229¿Àgì£VܱÀFhfýe
À:×+•°À<1œñ<îž@•<F,_/?þŸ°i¿·;?ÜØÄ|Ç%ï?Þùà@ÇñF?ûë ªšrÝ@áão{ë?Ûh $ã1¿ì;P8&¸¿ÝdgE‹%¿èIŽ;Tj¿ïÿÌÔY‰¿ïÿþÐñAGNbcuTXS 0310+022?ïn/†‹ô+?e!`(%Ú?a•7¥¨°H?a"tº
'œ?h9Ìdr?ŽßK²Â³?î~{æ!øF?«.ý¹¡?rQr+_W?‹‰pö˜»·?¥ÎXt¸?¨…ž‰ßÀƒ?ëöAÅp?£dÝU6?¥1yßP??'ÙfŸ!:?¸ç'ur,^?Ÿ©÷ќ5u?ìXÍ)éÍ?¡Ð·O÷?cÂúnl?_¦À@¬´Æ?¼ é®Ý=$?¡Ÿ†üUžE4FGL J0314.3+0620¿Êì+"4¥ÀDñLìAÝÀ:\¶wòÀ<:Š:N@ Ώՠ…ò?ün 9[ka?Ɩœúw*?½[$À?ôdõgö‰_?÷Տ;qÆ¿±§Ð(Q¿ê^ǀ݋¿Ø oA{P¿ÉWX×\»¿äíÑÅZ¿Õê€Ý
1²AGNbllNVSS J031423+061955?ìkuÿ]UÔ?¬—o´o?[³1…Ö?Q_hQª¢Ù?¼5ƒ>ýùY?¬yAèÃçÉ?íîH ˆ£¶?ª%B¦#s?}ºœù§Â÷?‹â¦ú
0ü?­d"X@ÌE?¥òôFUÚ?ìj9=B'm?Ÿ=è›Õÿ?—Ü4ÆFý?nÐ=ªÅ=-?º{:R«¼?^"é~Ç?å¼ù¯í?ª%wqk}?"xK¼>Õ¼?H!Úð¬7?Ó>ˆ$Ü7j?©ÆÄ5;4FGL J0314.3-5103?í=÷ßõôcÀJü©iuÍÀ9¨²ã»-À<XKƒÂ@úñw§Š@u_þmY?°S	<i½´?¤-?SR'?õ²`Š"Rà@ˆýµLþ`?ïè'á´,¿â±Ÿµ<O¿âtô3C#k¿Ý¸ãÁ…ñÇ¿âÖÑ"qïÜ¿Þû:]ôÒÐAGNbll3FGL J0314.3-5103PMN J0314-5104?ïï^.
¦?Rò<•ÜK?)ñ]nÔOç?%N®â‹?^x<ê,B?QÒñø{
?ïÇLçy?1Ã'ƒG?.)ìè=ÈR?Exé´B?{
%¨?€qR¯ ?ïCŒ­˜Ç?y¶'™s(?c>Â}#?Râ
M?•&¦Ô¬"š?x+ ÎY<?ï¦d.C?h~ÏzÿRÍ?\<ñOúh\?H¨rÝ*€?'ôˆÊoîÛ?f~Æü>ç.4FGL J0314.6-6549?ï
?§	ï˜ÀF¯mÚÎîÀ:ʘòª¬çÀ<¡öé	:@1ª‰€ò¯@')Àê?¾"ÛÍÐf¿—àõ@?ƒ?ÕÇ,#õR¨?üêõçÎ/ù?í™ö`ÄæÏ¿æÞÕþ¤¶-¿æ·é{Y<²¿åK¢•ÁÅ¿Úaf'–¿ïþÊ-ëÌAGNfsrqPKS 0313-660?ï´b–ˆõã?ƒbÁ—Óg?U	
¸†?Pő	nG?€F7œƒ"?'åÚÜØ?ï"ž1…ªX?"}^ŒI՝?R"I¹¾Þ?`²›ú$ä?š'õ3®Ç&?"¡¤1{?î^$¢½×?
Xšºë¹?€ÝÎ%§au?p¿pçÀ˾?ªâª,jJ?Œ¼ÍºJí?î◤ƒ­C?ƒsß×Æ}ö?y¹Jmø?iØhˆIŠ ?k)w¼8?'-£ºRNm4FGL J0315.4-2643?èCÖD"wWÀMYÝÁç–À;M¶Šk(À<¼½qåöi@!
K^"E?ú¢Ë;Óå?Él'Ê !É?Ǎè5ˆøâ?þD*Lä'@žq-êžð¿ïû—?ø¡¿ÝùV-3>ò?ïùÄýuŒ¿áaÏ}×Z¿àž+ϑ£+¿ãåªê#õ©AGNbcuNVSS J031527-264400?ï»ñkã§Ð?~fsè½7Ÿ?R4®Ž\8Å?x9Ðξøö?}zj•
2?r‡O°ôiÊ?ïbEË!Äu?–	Kƒ ?QôaÝ˜í?dlæüŒã?'˜'É—·?•;·Ðh?îœË 4¾?·6¼Ä·?vÛE•`?o¸ÿÌj?«*ʛ[¨<?Šàš<E?횚Û
Ùc?™cdHÑ×B?fšžÔ¾nü?d³ò§–?²vT0ëAo?˜þóÝû/±4FGL J0315.5+4231?»"Ǖ«MvÀ)¨Ût´À;lŠŸ*ÓÀ<—!Áçã@!rg‹T‡l?ôû…—"¤?ÜýŸ—Šv?Ý×(›T¯°?ø›ÌyÁ@A:¤Ék¿à>ÀÕó'¿å*øf®ŠÂ¿ê­Ù!nå'?µuc.xŽ\¿ãâÌ'ª¿äµðè5AGNbcuNVSS J031527+423249?ï/×·"å¢?ŸI€e©)?`k'៖ý?g$LnW?—÷˜±OY?œø‡á­Ë±?ìö8%`žs?Á¬ûýÆ?cÅã2gÄD?‰
p}48œ?·°»gÎG?Á™[%Ä¢ð?í+Bz6Þw?ž›®ŽœŸ?‡/Aš1?y.Hªԏ?³Å&FÆ"?›èõìH¿ˆ?섕ÞQ}É?¡hÓ±ˆ4?VnB@3¾è?WÜéåÍ;?»˜sB½?¡kŒÔ¤ð4FGL J0315.9-1033?æOÓï£3ÀJŒCoÁYÀ9‰ÞNÕP)À<8€eëí$@#Pn'i§@tpë$¦¨?± $"I+?µÈNŸ¥m@uûdÌ'@CîÅ&?°È`VìÕ¿á9äþú2¿è𯮯¿äŒ <Àü¿é/–Ð<¿ïñneZÎAGNfsrq3FGL J0315.5-1026PKS 0313-107?ïé¾v¦?]GZÏ+c??XgŸ<žb?6)𻆅?c4•rf)?Z±`;L?ïÒFf^Â?|¬Ð-ê¸?,€+ZñU?Gþ"¸+F'?uøÌ/•Ç?zf;ÀÍù?ï>årû™?|7þßÁ	?i5ë؜¢]?U»¢2§ÆÕ?"ü"%yGò?zß	òNY?ïëŸ ?çš?M¡U4ï?=M9Œ–a?0!ɍÑë?`·8æÓ@?I V'ý4FGL J0316.0-5626?ŸeC¦äÀI€Ç`|À;"¶Ò"mÀ=½‹ç)@ .ð%ä?õe¯ò¡r¬?ä=n q¥	?ä:ß%"å@÷üü?@•Æ1}%›¿â"ií£ù¿áß
váí¿ã‰Â@׶‹¿Êùá'çQ¿â©9êÝY¿ïÿÿ&¦³AGNbcu1RXS J031613.4-562545?ï´¯Žù"'?{>u;?bÌï½íÑ?\ÉóEòB€?|B,VÈÇ?y1v\ÖV?ï'ÑÎDT? ‡Â"ä®?b_jþ=?w¨µ'Ž9?ÙäJr?ž7Pßw"«?íqÉ&p?˜)q¢Û«A?
6I"¸?'®mêTe?°eØO$?"º#2‹?â__2?'?C'í½o?MßqÔ´ð?RïYx%Ö?§Cz\Bº.?';…¾9x4FGL J0316.2-6437?×ìéâԘÀG|"µÜÆÀ9êHX^eçÀ<3Ð&ô`@fyɹå?ùpÃLŠÆ?·N[ؘÝÝ?½û&Qxm¥@	›ü"$íö@ƒýLŒx¿ÒLŽ£ò8¿£‰9¥H­¿®·}bßÑÀ¿ÒŠ4¸Œ¤¿áqÊi¿×ÙFWÓ%¬AGNbll3FGL J0316.2-6436SUMSS J031614-643732?îïT䌑?"@aT³Õ?v] ÝÁ2¼?Á¹¢Ow}?œ†+þ!@?‡3¤¦‡›?ï,Vñ"??œ}õk€p>?UŠÓ¶>y?c‡È9Á¨	?™ðPT0?›"†~çM?í'¯_c–~?›C"ßX?'hÀ…?‡KÙ0¢?²êÔÂ'?•Ì£…—?íô×ÆE³«?''ûê+d?pæè™3¿Ù?] 5¥ÔŒì?®•¦ˆ~Me?'rœQŽó4FGL J0316.2+0905¿è¤vfPRÀCɤi×4/À8¹g«
fÀ;«ÇQbÉ@®Ô²?ýЕÊ@r?©`¢G'Ý?®õ|æ§â@¸G¢'v@9Äè§É³?ïöæç*F%¿ÙÐwœn¶¿Ý©·ôÎs–¿ÚCyÒSõK¿àðíޕL-¿àí¯e³¹AGNbll3FGL J0316.1+0904GB6 J0316+0904?ïÕÁÚä?j"ª 	,?3NV™¦?+€	å¤z?sê2z¤dÝ?j£÷«–?&Þ
d?‰{׺
€?=4TÆÜ?I{Þv¶MÄ?Šî¤rÀÉ?ˆ£h8'lœ?îÃó¾Š4õ?ŽS5yj·?oå"fŽÕà?du©6R?¡ÂqðóÃW?‹õ"9Å÷_?îR!2V}N?èU‰|#…?pSÏð'x?\™T²°¸ì?¨Órܕ&'?ŒvùRœbÔ4FGL J0316.2-2608?îYώ6þ´ÀLݍ%íÐSÀ9ÇøåY‹À<6@<H†@…[f=r?ücZ'ó+?µ\ÿ	Šî?¹s 
Ìã@Ì|Dôü—@PhÖ-H¹?Úöóý=Wú?Ïk>¬¿áŒY	†'¿Ð娶m¿äÕ\Rç-¡¿Ù›2Ál"AGNbll3FGL J0316.1-2611RBS 0405?h?zÃÒ¨?b}›,™?]ûÕ¨ØH?…  5p2?vâԈà_8?ï=žïز?(˖0"E?bµï÷?r2~€†¾æ?–+bËې?›е0Aö?í¿ä÷ô?˜Æ^™eýî?ˆuF
ÇuÝ?wN%æ¾?³û^§Q¡?•ð†ë6"î?ínXoG¾?'mû'×Àý?'Q*–''¦?|´«†®Ù?°8ñà#‰i?ŒÙ:Ù'4FGL J0316.8+4120?ê]X,´5tÀ+g0«¼²À:z®Žd•À<	›h¦²‡@"YBI-Æ?ý[8jª˜Å?È=º ¥Q‰?¾ú|2€†@Pÿ}¤§?ç:V[Vh¿íœý
y¿ÙBW}ë=P¿åqÏ ¼£Š¿ØÑN;Í5¨¿Ð¸
ãmx)AGNRDG3FGL J0316.6+4119IC 310?ïJs'5‡?•÷|P­Ž?@FMM­T?:Iž˜Íër?–,#Kæa?•¿8b•¯a?îCÈ}Èy?»Ñ±>r»?RS°íÍ"?fÜ«w7p?«0Ú¨EÄ?»£Ñ+…1?ìw-´×'?¤¨ü·ž?sWÅeÛÁl?i£º$‰*Ñ?¾fÊ;û‡`?¤eb.´8|?éљ ˜?±ù÷²²sá?h4~ÞÀÛ?b<~»ªÅ?ÈY"«Æ"¿?²'ÙúÇõW4FGL J0316.9-0625?ïSCu÷¢ÀHÞìAÝ"À;Ÿ†B¤ÀÀ<©ÓåjS@ "DðIÿ}?ü,?ùë	?ÑA ^Y҄?¿¬œU¶•Ô?íÞ½ý&1@aÒ"ø¿äEå½_¿ë5ßàл¿Ñ«±EX¿ÝÒéý	U"¿à»ùu¢CŒ¿×]cß#'AGNbcuPMN J0317-0623?ïÉÚí¡I?}6Þñم?0ôUVú?&£ÿH¶d¿?zMêÀ?}†—Ý&?ï{hՀ?Œ%º?@Þ;ëÌRó?QM¦*€¸?¡æíl?ñhåj?îT‰±ý?Š2nQȧ‹?hýh	)¯?T¥_Ýþ*Ã?©'Žn°<?‰'K¶D}?îñŠ%W}?ƒ"-ڐ'?DÑA¡ª…»?9"ñKrÉ? "ç#Þ?ƒw˜à*ã4FGL J0317.7-2804¿ïS©Ý€ñyÀLÚ'¿aª?À;ü/çCÀ<Þè	i5N@A`[	ø@þãþA¹ß?Ótá¾ÌY
?§ÂIÇI?Êê›ê¬±¤@pM
ú¿y¿ã-Æèl¿Ý¢}ÃÐ#ï¿çòbo¶Ç¿áhœ|&¿å#ßYw¿ïÿÆߢèMAGNfsrqPKS 0315-282?ïÌ(a‰ž?pÛB éÑ?A¬Ó;Y	à?;þ¦©þÃ?w¶4ԏ'?p4]?õÇ®?‹Z˂û¬'?@s慼܆?QKXB"?‰Ò"72F\?Š:¾ÇÍÌ?î#8—ž›é? Wÿ. ?{šÑø@í?tB[¼ð[&?ªYGYY?Œ£w»}ùc?ïy^$¹àÞ?vØ]·…ŽÝ?<ÅҀÇ?1ò²-¬A'?a$ö+?vÞÂ:©œí4FGL J0317.8-4414¿¥Ò¯6<gÀL´ûß	À;¡óQ›ÔÀ<ïq"§š@!wi¹'G?ýnvÖ 2¥?È0î	ˆiñ¿Ž/¹gP'?Ç?·e‡nI?ý\?r±£?ïø"à4ê¿à L jÓ¿ç3f"‰`¿Í›ÅÃď¿æ¢BŠ"?УßBÆ#AGNbcuPKS 0316-444?ïT®£;üZ?‹ñÓ.Ú$?>-ì~ê|2?3ûQ‹\³¸?"ñsæ"Êý?‹°
¢fÈG?ïJ‡õŒ?¡?•pêû?T'™"žÜ_?cSˆ=±v?•e×µ>$?"&åÒX?í¢²–îœ?"o
¦üæ?p'@ƒxB?`Íy(ž9Ý?°èvcc¢?"¶»&á~~?ìø~‡­†ê?¡bý½r=?wdbþÚ ?n"[ïp¤?¶ÅŒ¦§?¡À8'¿{4FGL J0318.7+2135?ënZ‡q41À=¢Ž£œQÛÀ9{¤ÆôFÀ<˳È	@ÐõØ´·'?ÿõ±]½Õ?´¨ÜW¯>q?°¥¿AÉÎì?û‹ÐÚè@	T¯ƒeД¿Ùs†Ž$¿Ùv€d¿â_Ïoº¿Ø|10É¿åE!ýÖ¯û¿ß
Ë |âªAGNbll3FGL J0318.7+2134MG3 J031849+2135?ïÜ^Íx³‡?ju
{Z'±?<QÁí¹:Ì?2c•/
?p}$ʨ?hôÅCt;|?ï"Ý…È¡?‡ß4-ñuc?@'
žTéï?QŠç€z
?‰ÿ—ĨˆÓ?†©˜¨0?ï*Ü=žk?XC"‹µ?f"3â…QB?Q'Awš?—ë]ûûˆW?}'¨³§Ó}?îð~Dìòç?˜=i®‰?rÓ·uë?\ã'^²z?;I… "Œ?|–v¶´XŠ4FGL J0319.4-7045?³jÛ¾r»
ÀDÕa^¿¨øÀ;TÔ«¾_LÀ<㤢â¸@ ÐtcT8<?úW£öíô?ÏûÉ,9?ĺH¦7Û?÷Yn€ç-?ükà£Ä¿ççΰқC?âÞ¨—c^t¿Ô›½ ´ëۿ܌"aFA¿Îº…@q4¿épTü±–æAGNbcuMRSS 054-102986?ï/ÔQ?'"ÆíŸ,8?W8|‡CrG?R&5ZêîÃ?••'>¶?'"ÄÜʆ?ï$jùu¥€?"‹ÜîûX?Q6¸‰ô$?]SaHŏ?š_5H¬¾?"Ü0>:h?íú†^¡;?Íh8¾Žš?s|äD¸J}?c(þ‰é­??­èK~ã?+KLµõ®?îCŒ†ï-ý?Œn11å·×?h‡£Xs>í?`
«'Ýæg?ª>½[…ìL?‹ÛA}4FGL J0319.8+4130?ï@ÌÁd8åÀ*" _ñØÀ5Ó²Jj‡À:H¡¸é@oÊ·sÊ'@_&DÉ^?"sÚ Ó}I?°œ}#Â'@'<-ðÔ@ ÷½1ø¿Ç>¢Q#¿ÚáÚ»wåÀ¿â#%¿,P@¿áe°ÿì·¿å`ð
j¿æE~ßÙïËAGNRDG3FGL J0319.8+4130NGC 1275?ëhÀ ›Q?¼4I•B¨F?[­.|U©?_:r–*ð?ÇÑ š?¼ ?¹òZ?ï_Pt8ˆN?¡…°£Ñ÷?gMàÇÙN¶?}¯Fª®?',5_óÌX?¡	{æþ0Â?çàò¦ã…Ñ?³S͇g-?¢)öÞÇd#?™_Ü0ú4%?Ëñ·¬À´?²V]¿Í¨?ïN£ýãÓ]?‹~08Ù?YA'&B?YÒӟoy?"—g!$08?Š›eïÖ§4FGL J0319.8+1845¿ÇV—%öߛÀ?²Ë…¤ðÀ9ârkWfïÀ<
øGv@!xH¥á%Ÿ?ùބ 
Q!?´½cù#ÂÓ?«³4uR't?øšc
»@;˜Í@åù¿ïöÇ¡Р¿–<¶áöL?ïÿÂWþė¿Û¢hu4¿Òܞ¼n/Þ¿Óg/x°kAGNbll3FGL J0319.8+18471E 0317.0+1835?î˜E¯IÔÝ?¾çÇ«¯sg?Xκ²Ï
?pāMÇ?¥µ1
Æ?¾z#Êìæ?ï»ÜP
»ò?ƒ¹¡Ãù?'c½6ÙɈ?@Áð֊" ?€«]uœn?ƒC'X:ö?í2S5‰¦?¡t­»ý?dÅsZN¾?[pÔNªÐª?µÅi˃p`?¡Œ,\ö?ïZ?ä@=À?€isrÎ)?5þ­ ;ª?5xo<"Uf?"`Áw[²?€`ØW¬_4FGL J0319.9-3821¿ìtóËû<ÀLˆ¦ YŸÀ:×ÜhKBôÀ<¤vtÑc5@JëêI_o@šތò?Ã0èU>v?¡"!ý=$?Ú'Òûº÷@	EBҍ?ïç/ï±Ô#¿â'eÀ¤"¿èÙà[DŸ¿é‹¾dª$¿Æ{ò>ÌC¿ïÿÿ" 5•AGNbcuNVSS J031957-381527?ïæ7êê˜2?dh¶éÖ)í?9´CðÁ ^?G i"ؽÖ?f'Œ—O¨'?c˜ó9 ;?ï›/[1§ë?‰ÿf{î™??®"2ì?S§‰"0?ˆ6¹'u;Ã?ˆ²«ÚäŅ?îçrÖJ™_?†Š8¥Ù;°?i­_=¤:å?a9Á,L{?ŸÛùNøLâ?…š«Pšhc?&ñ§gŠ?iêFšã®à?:o3"Éi@?2øiÍã‹1?€
ÉùÿÑÅ?iKºŸ¦ÑW4FGL J0320.6+1125?À¢âØý²žÀB¤WÙÜÀ:·ŒR‰9ÐÀ<õ0™%@ Wò ò@… æ"ôï?Âó"`›2¿¥>" šœ?âhâý¹÷@2®Å$⸿Áe¶}ªû—?ì=ÙI²Ñy¿åç-É¿â(<县ⴜ>ån¿ÑXü…÷ü%AGNbcu1RXS J032037.9+112503?íJ»"A?«™Ä¤'?'}e2L;?}äÒýýûî?³`På}l?ª²µ¦¡T9?ï•ä¾†?•?3*I¢?R‰¤škæ_?YçtM
Nw?d©—0ú?"²^¿óÖÏ?ê©qùŽþj?©Ã&ŒR ë?a²ß'p?w'rp€Î?ÃdëÓä?¨JgˆW`h?ê,·$êƒ?¡Â4ӓ4º?…WVù?x¸z§÷\Â?Å÷³
¶ô'?¢
•
¡£4FGL J0321.3+0425¿¿š`WÈW·ÀDÿ†ã´oßÀ:§S³ÜÀ</ý ª/@,ÂìÏ º@!_Ìr?Á4ˆó¯¿ª3j¾9?ê‹ÀBzÎÓ@äÉ?ìºåC¼s¿ç±à¸<¿æÏu¹Nk¿á|øCsW¿é&È÷U6"¿Î÷_]ÂíAGNbcuNVSS J032130+042628?ì¨Ñ­GV¤?³Q#ÅãÞ³?"'†¥ó??w¶öû3?¸4Áâý?²ÌðÉg´Â?ï	´°+÷ê?™ES¿Ï¯Á?W…"êµ?j|hsNÊ¿?Q¹bb?˜8©}s'Q?í/äÑdÿ?›ƒ¢¾TË?…2í1§Ó4?uiõ	[4?³Ú{ΣÍ?˜" È0
?íêb·€ƒ?¦l-£ÆÈ?rÕ%­"Rø?aQ¿äéþÌ?®ÿ/ÒGDq?Œ7ÙÖ0n4FGL J0321.3-1612¿ãë–Ñ_¥úÀJÕf@¦¹=À;p%FáeáÀ<Ä#G,å;@/ëîÑ?ý橝ÛÙ?ܪ'zÁg>?ÔֆŸkë‹?ýÕ½6VÔ"?úBöt»ê?ëw¥ˆ»%?ï°iŠU_¿áj¿ÜÌú61ë¿ä,HÐ(¿ïù"O¶!AGNbllPMN J0321-1612?ï@M¬â‹é?9EÜpO¯?m³§#·©m?eö˜­P0°?"?Õ7Õ?Žƒ®Íz‹?íó 
í% ?­Â"ÂÎ/{?†d††û?žf6Z¤!?«>eÿ§ŒW?¥Üovü=€?í¿?˜+cíCû?"»jÊ1EÂ?"Ôâï®É…?² )T}¶x?"g¨$m+c?êÕðdrý?¦ã©);WŠ?"×€»n? š°Í‰Á?ÂGd®Þ£?¥øÔ߽ƕ4FGL J0322.0+2335?ÒöÄK¸©ïÀ;˜§'h˜À8ßaúÆÛÀ;М·[K€@^æÀ=ó?ÿƒëaãIç?§uëƒ`?‹~Ö¨KkÂ?ãYA¥Ã@øù²%?ïô5â:\¿àñ¦ é4¿âúúÁ»¿Û'ýûÉ¿àÃhjL¤ô¿Ùº å¾5ZAGNbll3FGL J0322.0+2335MG3 J032201+2336?ïLøh™?Œúˆ:F"?R5Ó¶<?I'5Èa<?•=¡=p1Œ?Œ€

Ò?ïâžÅÄÝ?Œ7œìà÷?IØtÏCj˜?`çTC—%?éÑš'!?ŠAÎ@ö?텄¹æ<C?ÑÊå?ƒ¡ËöϧÕ?}Ð;ß¾"?±_ ±ô(ä?›'ú¢&ŸS?î?½œÙA?ëT>Y5æ?'¶-ö4B˜?mõ™Cgà?§VšÁU[B?§‹¿=n4FGL J0322.4+6606?æ<rՓ#@Teè'%1À:%½›¡æÀ;¥KJ-'@Ri|ñBM@TÓ¥¸?Í%ÑuÓì§?Â(ÅÆôÄ?÷¡w´l"@mËÑ¥#»?ïƒß=g¿'¿ÌŠ|ºe¿ç
@/p¿ê¬t½—$ʿ竊\å´$¿ïòªa½à AGNbcuLQAC 050+066?î{ñ2«¶p? ËëÈñþi?UÄ=2x.?Q[­m{?§'Êë°ØE? ¦Ìîǐ?é'^®>Kz?Åò]Æ<¾?xGܧÝÇo?‹yŠiì¡?Ê FaÇãß?Äv³Zæ?ê¦ß¬'¿?§Zˆ»QeÐ?–µŠÜ=ä?†u;@ùE»?ÅMÏò1D?¥W3¢–œ?ìÈ0¾*DZ?—ÐeÌ£ç?yFD
™ø)?d`¸þø¶?¸*ÍÐ"÷?—[Ù%?j4FGL J0322.6-3712e?ÅùGÿóìÀLX±mÀ9ÍàöO}À<Oʪ³Q@ÇìÀ24±@9‹q¸ª?²ðìçŸ?¨)>'·Ó?ö U?Íui@¨ÕzÆDÈ?ïZeÁû¸s¿´åcË+¿â³KQ7*9¿âÇÿÞr¿¿á>ÀÚü¿ÝŸœèÙrÍAGNRDG3FGL J0322.5-3721Fornax A?î'Üan˜#?˜ãû@ó?eÓ¸\ƒ,ù?XKL#
?¥tþcNJý?˜, ÿÒÕ!?i #?¼vò®Æ:?I¹Í,vq¯?X'çA¹KÚ?Œu]ÒА?Œ;«ÁŠ?ìúT'­Îˆ?P›³՘?Šÿ3‹U€K?¨Ó(l?´Ítù&Û¹?™K¥¯	)?î·eˆ]=D?ƒ¥›ƒlP?~æ!«ÏEs?iõß"y ? ¬ãD²Bù?#fím4FGL J0322.9+0940¿î@g'û	ÀCŠ'¥aNÀ:ËW´ûßÀ<$ý~E€=@òÁ	J+@1fàé´?ƑཚÉ¿_Œ‹Û?¸*žd.©?ÿ›£4"¿î
ÍHÏD?ÌfH'ZŽ¿æs½œ®!¿äYQªí¿á.¯½µƒ¿áìà¾q?]AGNbcuMG1 J032256+0941?î
ªi›ïÃ?¤^ªF5?iڗ"<rõ?c^¨/W ?­·¯ô<¬?£ë"¹5é?î°Ê-ã:?¨ÊfxHuJ?Z•
¦‰ý¾?gA±'G¿?¤¶Ïí|m?¨'ºé®+?줛N™??¢Fxrû6?Š©#™í±?z?]Ÿê€A?»½¶²M"È? së8¬-–?ë|Ù,§â»?›ŸÏ¸3?t×êeÀV@?hg9¨+Ý?ÁeÛú2rb?›h4T¬G4FGL J0323.7-0111¿Ï»؃hÀFœÙ¾L×IÀ9y|"MÀÀ<ýð[GN@²S~'<?üöñý2Æ?³†þ6|>?¹ œ,ÆÝu@ª`%څ@ã‰û÷Þ?ïÿ-<y-¿ÅƒÙ¾Í±¿ßúTvyÚ¿ÑyzϪ¿å†Ö]ð 9¿Õ•:¤Á•âAGNbll3FGL J0323.6-01091RXS J032342.6-011131?îÝåñµV1?"Q#iUW?k"	G-û?pEy.i? o€P7½.?'Á,Õ²ø?ílePlî°?³ó1²©}ã?Néx?¥¯óGFy?°ó8Ûi÷?¬­«òÊ.¹?ì˜NNƒ?¡²0ÈûÏ?®‡IÛM9?€*œÁNž?ºï›»ø¢?Ÿ½~2žïÜ?êåšhÏ?Ÿ‡¹lp»?£uÇfÍÌ?ˆ%ã×'²?ÂðL$†-M?œ¹˜¹'¹€4FGL J0324.3-1313¿¹ŸÝ€y7$ÀIÙÕ<ÝÖàÀ:ƳÑSDKÀ<rºÇË)@¾Z.t²"@l'	Z?ÅÔú˜¸?¥CÃW®?àLS?È@f¢$'–H¿Ñ-!¡:wË¿æ<¿ß®Q¿ç/SàQäÏ¿ã§CÁð`¿êÖ
ˆ~¿#¿ïþašNË?AGNbcu3FGL J0324.5-1315NVSS J032430-131002?îøáùxo•?–•"ø¤s?kÁ^ˆ‡q?aSzÆÉ?k"ÿáú?•€ã¬)Û?ï]&.-7?'Šô§Õa¢?GÂãÑE"­?Ub†nÐ\‰?"#Îò"?õ1àŸm?î.:Jr?ô=BÇaÄ?~ŽÊ{äà?oÑf‡ÓÒ?©ZɄùb?Œ'îõêÏ?ï4\(F?z»mÎ.²?d<kå"{¼?Qbý(ž?–õ¯wÊg³?y%±ÿ›€ÿ4FGL J0324.8+3412?Ì7ôß¡¡âÀ2¶®::ŽqÀ8­<Íè«À;±5WСn@—#ȇ@)@k*?¥ ‰ª
Z?­‡½Úy?ÿÉóÔx"@#ò‹ù
¿Ù뎃æÔá¿çöÌ ,/߿ꉢ«'â¿éSÐ↏¿îcó¯5?äÆ@–žAGNnlsy13FGL J0325.2+34101H 0323+342?ïñªÛ¤*?Y—ñ3,É?;¸ ,ÖÐ?6§¼x{Žî?U¼AîìyY?W—ÅsÜ?ïÏÒÀé¿%?~Í)Jó_o?1ñty×âž?JàIï3×?v÷ˆC'ð4?}·m¯†/@?î…8¿l?"B¤23ø*?€`B§íZw?|²Ž€‹?£"mº
Ҕ?'OµÜ?ïé"ûšï?UÏ+¥á3¡?CöJRÊM?:ã´üÓ?aìJo²~™?S±qËf4FGL J0324.8-2043¿ë™ó±	š*ÀK?™ÜµxÀ;hi²KAGÀ<ÈõZŠ@ "¤Ht8?鏂¿b€ÿ?ß>P}pï?îøÒpXƒ@i΀+3Š@	î…äÛâ>?ïùÈþáòÏ¿ïñ"ݝ)œ?ëÈòíÈÅ×?µnTœdz(¿åvpnö¿ïÿÿ" 5•AGNbcuNVSS J032451-204324?îX"&ô•Í?ÀDbkœ?tÀ¾»6Ÿ?ÿî0ÀÐ?§åŹOÏN?½'ÑZ=|?ï%½ØÐïþ?£)-gØ^?euF¶?L
ÞÊÿÏ?˜™¡SÙ)T?¡/†‹ÇÀ!?ëúd"Oó?§i֝6â?ˆ‰c:6˜•?ÀÒ..‡Ì?½¯v@­V?§sACœ?îA8"ÿù?¢á‡:€Þ?AD\÷¤?Bsìóø}?«©ËÒÕ?¢êÿ´~lB4FGL J0325.0-2416¿ï›ð›½ÀK³w ÈÍdÀ;[s¶±•À<µ\ÿµ@ßý®ÁôØ@]SG¥°ÿ?ÂÔé¦Í3пµ×"z,?òã<æ:\@hNAy¿Ìb{ 4hg¿è÷ÿ¶.$Ö¿á•+uϏö¿ïì;ýÝ?퓟ïôð?Ì7
Þ:ŽAGNfsrqPKS 0323-244?ïÓ@鴜Ô?"Ó¹1n?5W5¦.?:G%'á,ê?u
âW4R?"OD|ôåã?ïNúuR¢^?¢qFZ©a?a)Ç<5?~¨þÇ*v?"ûxn*3ñ?ŸœmÓr£?퇵«>b'?™®"ƒw?x¦+Ð9¸›?ro®¡žÄ?²7ïé	S5?˜.¾§æÞ?ïÔ6oó ?qÊßÆéL.>üºU…¿?
v:u=Ä?uÈ
ðà?qÂõ×Ð4FGL J0325.3+3332?åkÝðEÖÀ32|EÀ:ۘkœ0MÀ<(ŠÅÁ@@ÞÜØÞ}ú@Ñ1ìVu?ο'½†,?¾¡Åg}¾?ò¢}SõÌ@Êãés÷t¿ïð£5úÐ?ïýâƒî6ª¿ê¾ÝöÀ¼¿ÃË`æõ—ò¿æ£Ò½§•Ü¿ïÿ'ò¶kaAGNbll2MASX J03251760+3332435?ïqˆ5?‡¥ðJ­ú?iÇó•;£N?iîeN¦v.?H!ãÓ)?"Ÿ15k•ª?ïl¨Ëai?"©V-PI?S‡æþ$?c""]Í?'2h>cñN?"Q‡›¢O£?ì	'4"V?¢S`jk!?‰UÂ/´R€?xW¢i{ó4?¼‰6èŠð?¡¡QqºÖ?ì̟	 '2?›`==¶¦?‹¹Í"6·<?}Ž~¡õE?¶#ÎtŸ‡?š›8¤[Õ4FGL J0325.5-5635?é†ÃѺÀHé*0U2aÀ9ÞT8fxÛÀ<c!¸·l@¤&ó?þä¡Õ¨>?²@ÊžUì?£Sþk«?òTE·š5¡@´2vÐ?ïÿ˜ È¢q¿ß°Å/Iš¿ÜÚ\FQô¿á3ËÿY˜¿ÙÏ:û©"¿Ü£¸AGNbll3FGL J0325.2-56341RXS J032521.8-563543?ïæJ´ñI?_»íš~=­?*@‹ß`Jp? ~9…u'˜?hC3±?^œœ.Âï?ïĀðìI½?€–‰&œr?+fë‡'ÂN?D˜:S?|äP-¡ã?	nc¨³?ï
ÀÅ
Š?"?¸ïÞM`?ffQœ>cõ?cq\Íû9y?›³Ö'G?ƒ¼S©z?ïµH-E•?euŸvb¯1?Gˆß·L¯?6»Mďû'?5x6³%Õ?dƒhýþë4FGL J0325.6-1646¿èøáZð´ÀJwÃ?…Q
À9'BG£-À;æ³ «Ü'@¡ØR¼æP?üÖ#l?¬bjBD¸?ª—ÁA;J@ìsƒ…[@
sd{ª›¿ç=†É2¿Ôëˆy¶¥C¿à-qÊÛ[¿ÔOóÞ3§w¿âEœÂC¿Ñ,`Eºõ4AGNbll3FGL J0325.6-1648RBS 0421?ïä˜0Èl?eoY'JôÑ?'¾{û
†?!"%MÛÀ§?iëç†dMk?d­ ‰ÿN?ï¯Ð†µå›?…óŠ¬8Š?7ÆTI¦×®?O7'ƒï¤Œ?ƒM«°9bÛ?"ó{R?ïb6 ð?ƒ5N] ²œ?g±±–Ô¦O?WŒ1ŽIH?›ýƒ
ÁLù?È<šö"2?îø8)h7p?K9Ú'Í.?YûRYv€ø?HÿÁ(k´,?ŸYE­a©è?€Ãh4ëÞv4FGL J0325.7+2225?îkÆ£ªYÀ;ù@»±òVÀ8¢ÆÅKÏÀ;Ä"Ÿg8ô@G¶h‡Rð@K%}h
«?¨íöëÁÉ?ÅdI,@öøj	‰@²ÑÖKý¿Ø1—׿¿äª¿_»ý¿èwÓ«äù¿ë,L$Ì¿íîa«ì¿ïÿíöé	AGNfsrq3FGL J0325.5+2223TXS 0322+222?ïÏÓ®²?nßQƒ'‹?m¨·Ä<%@?g°Ý†Ñ¸˜?bƒš+Á)Â?]rÌTµf?ïÐp=(G?­©>Y5É?tÇqïkÈÀ? HJuœc?—4|€Ì?¥ˆíË§?îŒL3èVi?–±.Ò?"öÚn#ÎÇ?ÆR?ò†Ê?™ŸÑcú?Š¶
æÐÛ?ï\p$[ÎÈ?}~ê\f?~Sтpt?pKÛÆlj?‰ºhKÀ?u'/Hµ
:4FGL J0325.9-1843?ê'ñ¹|tÀJ̹#¢œxÀ;³"â{À<‡¡†`@aA¹^@£BàO`?ʕΈ䕖?ü–"¨q?×jîöÃ@\@c±^²<ÿ¿å‰ÿ]BÑ6?ïÁÿáø¿é. À4
¿ÕHãß
>¿è^ëÈRj¿ÔX£š¤["AGNbcu3FGL J0326.0-1842PMN J0325-1843?ïŠ#ãÕR?ƒ'–l)8'?SØ}MWö?U™˜'?Šü/g˜?'ËûD-Þå?ïÂe|Ì?€l8JËh?$½Û¬›.?5w4ªžÉ?~-<œ54?€¾Æà˜?î&H£££ß?'b'!ñÕ?t·Ô'ü?fÛü¡
æØ?«{@áþK?ÿê´/›?ï~ºIi/<?sùpoƒv"?ZÐv¤˜l?LV
h%ҙ?3–ßž-?sM¿ª­…4FGL J0326.2+0225?½¢™×ÀE5¬îàóËÀ9RÁmóùÀ;ý'€ ¤P@ )j \×F?ý™SÃÌs?²ƒÆôp«?"¡q\í?îFTþ_@:;j?ù?êEXßÀ‹¿áp^¢LƂ¿âsEaÞí6¿Ô£,å¾`¿×²!vrM¿ãûbâMhAGNbll3FGL J0326.2+02251H 0323+022?ïTóKí²+?QzGé?Qn(…'?Fy'0Ê?"J´Ñg2Z?W©‡îXq?aHF?†]6lê~?5w`§£?Fs'"Î4?†õWl­iq?…›·"JR‡?îbYÝÄ?'i¼	!ƒ?q¶ÓsLó?a<uÁŦ?§¼ã•cº?',©V­'ƒ?îL8{Ñ+?‰4…e€ðb?ldšŠxÐ?VýF†©°¼?©v.šH{P?ˆWÿVæd4FGL J0326.7-3404¿×0òš¢êÀL	U`"¥À:ÖõtŒÀ<Æ$)ªô5@^ê˜Õ?þb,•Š@`?Æ(¿ý0—Í?É(Äûb7@C]œ"I@éj£·Õš?àMÍþ¦
Æ?â$EÅ.…±‡!¿ÞÉÖço¿ìÏ‹¿¼¿­"ŸÚsAGNbcuNVSS J032644-340330?î–ì"¨Jß? So/?ˆ­€å¼ Ý?…1©­Ø¶¸? eݜ)Ô?™Ïx•XÇÿ?ïgZ¹¨Ý·?'SUdÚ«?W­D÷p}?l8ÒxEÍØ?'™Ô{mHÏ?8
*cõ#?íyíÓý±?—®ÍÏÎÅ?–«ù|Þ?ŒÄÉ2{3?«ÒddwµÍ?ÆVÞb?ïg¾4/Ñ?~Å«-@‰€?y௠~9?iéßw>õ?–OP
±æŠ?yh±s`	Þ4FGL J0327.5-1805?òÒߥÀJrGE8ïÀ9þ\XÆj³À<3ë‹Ô´ù@ñÓ"§IÛ@‹ÞZ"ÊM?·Ý­DÇ/T?¹@1¸#?õõƃÝp@Ä E°8m?§9ÓtÝ¿è	N}'{=¿ìòwéF¿ãˆ$&Oõâ¿ëñ–¼ˆÝ¿ïþùÀJÞKAGNbcuCRATES J032743.34-180342.0?ïô'(Ež´?UaP¿pp?Jb–Ï<°X?LžÒrȵ?EÈH}›?E9üL–%?ïÁ]ör¶?%ðƒØöc?2 ÷ãqÎ?Eù"ÿXè?~'h†‡Ï?€\Ôm³Š²?îúO½}ù?ŽùLgwAÈ?rQº–‡l˜?qÛ÷ˆÆ¿&?œ!™ªŸû?M´dyÜi?ïâ.'àś?V ðFՃç?KÎ¥÷¹ ?@
""ÕŒ?fÝÓ»¼tó?R´8£ªS4FGL J0328.8-5715?ØÝ[p5rÀH‹¼¾aÐÀ;žJœ	¶À<ì^ª°BS@"t˃÷q?ñ×ôH;Ù?äoñ•1ä?á—Ïà'~@˜"?úJVËhɘ¿ïå¿Â£(9?ï–Á¥)ñ¿äÀ€æDm¿Å3ÃçJýT?¦à±[,K¿é}"€U$öAGNbllWISEA J032852.69-571605.5?ï"àFAn©?—¹3ˆmj?k¦QŵN?fÓ>w–2§?˜/,ÿ/4+?–‹ö‰¿ã?îæ‹J""ô?¡Žú§"'—?i¶Òͼ+?"MdQ>.?Ÿ÷¼k3©å?ž¤ö´«ùØ?ìÚ®1,A?œ(g2úÕ?Ö˜ð&g?'óAËæ?µ/»Xœ"?˜
ø,Íc•?ìŸSÊ]Ñ?£÷õu—6?UÁŒÙ›?c8þ±¦?z?º°.H¦ÿ?£ø×¹>4FGL J0330.6+4659¿Ã¹TæÐôÀ™tNƒÀ9•¶åû7À;ÀcK(ó>@<8?Œˆ@oÐ!ëã?¾ÿ·ZʦØ?Ä/â›Á-@Ɣ‰`[@g+Þ*B¿Í—£ö¿åz¡–'õ¿éÎÚÄT®¿éêÿR[§¿ïóȟ@¢‡¿å¶]õ~AGNbcuB3 0327+467A?ìö¸×É°¶?±éËÒÜÀ:?}GÙ¸?ŠªºöQåM?´C™ïëCß?°	ŸBˆ?◌cQLÔ?ÎüÄçÐ0=?™,>4,µ?¢³O®'k?Ù>#V›?ÎOÁ*[ù?éA
ٕWu?¬ÆP)ÎH?¤Íå{

ñ?'ë_V¤§?ÅÈ[:ç^°?§y{®B?êZûÉ?O?¡ÇîØG"?ª/µYÎ[Q?'¸ü×V8?À#…Ckô?	àð׈©4FGL J0330.6+0438¿ìÙGÿóë ÀDã>ÿPÀ9Ï"M1âÀ<%E«Hï@»ƒú @DÀßXÀ‹?º½<áÝ«?¿C¥`$Õ@»­À˜$@十×?ì۝_¡Ñ!¿´&,9™Ô¨¿æŸ³%]¿Úþ$þ½	á¿êý՞,¦Q¿ðAGNbcu3FGL J0330.6+0437GB6 J0330+0439?コêƒ=?¢Ò%›ócÜ?\@Ñ#þ'?}Ó:'¿Ç?z¼Ãµb'?žM.?Uï?ï–Ëk×í?Œ$ö»ó¹?D>Ù:Ö^?fk2«M?‰	7¥œ¢š?Š>÷Ú²?îQ<"S)?oUÜå…9?†ÕÏ#è=?'›Fàµ? uxn÷G?ˆ&ÇãæҀ?ïBXÖäoþ?zŸ"˜6f?mŒq±"?\Š8#±Ùk?"d•O‰û?wåþ'þ4FGL J0330.7-2408¿ë½š£7…±ÀK82vtÑÀ;b«ð´2¢À<Ù£€£(@ *Ï·bØ?úM "Ú?Ôä< DXŸ?Ïpk"ð(?ûãèrDÁ@ƒ¼|±¿ïʒ€Ê÷?îrE ¿×¡P&kú¿ÒtZÅÉM¿æzÐKŽ¿Õ>ê šªAGNbcuNVSS J033050-240612?ï—øªüC?ƒ;|=8¸±?S_¤¥©µ?IYVÃÄÀ$?‡•àé]¹ß?'³3bWu?ïCm>
³?'‡Ï^ÓsÖ?U#fÇ)†˜?bƒ®Y¿O£?–@%ëÌ6?'–Ð8"¯0?íðÍBšb?'€ÔRvÏ?€B• 2?pÖ^î)Të?¬í›Æn9"?)ñÙp?îêE$®ž?µþÝÏݐ?n¶?>%Ý?d¨Ûž`Ž?¬¥÷¹Ì#È?yÇsËQ4FGL J0331.1-5243?áµ·š4äÀIsüC²Ý7À;&ê«Úä¾À<ÃNÂò®@H‡r¦@yýåsŒÀ?÷øX$Ú¿š÷•ì¼?Ô©S æêÛ@É(Åñç9¿ß˙‹í¿âþP",O¿¿é'A¦"} ¿àXÍ¡ˆü=¿ïÿý±q&´?äQªí~ôAGNbcuPGC 013066?ïãA^'–?f=çø#t?K—=±Òy,?GNζ7×%?eÙ5˅?bʌð6µ?ï‡ÜEÖÿÂ?ŒùûÓÒø?D°Ð/áŒ?W•;p6VS?Œ½á‡Aÿ*?‹Y霤-?òƒ3?Šº 2Ã?v>"úQz?i{1Ni8B?¤<"ž'"?ˆË}"µ«h?ïΟ	 _?cÞhۊøk?HïbÐ?=¹°o'j?u­O½M"@?b­ ]ÉÞC4FGL J0331.3-6156?ëÛÀ8GwÁÀG(µÃ›Ë£À9Yėt%À<Jè:@X+ü2@?ÿbBw†?®™½
ù#?°êÀŸÃ@¥:œ´M@¨]e‹Êú¿×û_1hÙ¿~‡€££¿ÞÖtD¿áÀmä	)t¿áæ!‡+¿ã˜r‡ÜØ´AGNbll3FGL J0331.3-6155PMN J0331-6155?ïçL²â?dy»ŽãÉ×?3¼FDž?)þs´u?fj*‹z•?cÛ gqc_?卑±B?‰·¹k?™ƒ?;]R|d?TRˆG&yí?"ú3©šù?ˆ,g­Ý¬ø?ï.‡¸íœE?¶ù•ßT?j['šô| ?fëæãÊj?–㘎íçÃ?6rDº¯Å?89`&?m–ΧB7o?b™ö6µQ?P3ÅivZð?…ÚKtIW?jYœoŠÓ4FGL J0331.8-7040¿éâí±¯÷ÀD{tÝÛÀ;ç&ďçiÀ=©'^aµ@"ÙJb¤ºà?Î*ÚI7+?ì?»×²?éóœDnÄÚ?ýâ©Ô#Ù@í§d2"¿ï÷[0H¿ïOµIùHV?ïé !óð¨¿èÝV‡Ì¼?Ó¢=ëó¿ÊAÜCbUAGNbcuSUMSS J033202-703952?íø±F?¾wÛõñaŠ?|=i:ªd?ŒŸ©•úÍ?µTcåœS/?½Áù€L?î¹0ŒA|A?¨I?UŠ´ ?li®JŽñ¹?ˆôGH
Gê?¢¦\W?LÛ?¥õòJáØB?êõ^g‹?§®a‰z2T?	"Ø5x?VäãL?…?À‡ISÆÍ(?¥ívGw¢G?íFÈÞI?°ÖA'\Ï>òÇX;‹­¹?ÏÅ@6¹?·¼JuTý?°ÖjùEgÈ4FGL J0331.9+6307¿Ã•žð©@Ç€¾À9*æ?d™ÞÀ;ÎÔ°ÆÜÉ@×ÍKͳÒ@4dÁJ¸‹?²vNÜ±œ?¶Mp÷ê@WZYèª@	¸¡"Ä"¿Éëð¾ïi…¿âLð=ë¿Þ[^Ëgqÿ¿â‰Úßµ¿âú1T5â:¿ÔHþ¡†"AGNbll3FGL J0332.0+6308GB6 J0331+6307?îR³ºµî?¤°:?aÁ}-ýë?ZUt"ºæÓ?©¸¬"ž>ò?£q¬ôó?èlZ³©?Ãu\xªs?yÃ|À‰\?ˆCܾ?̀|Õu›O?Ã:¼»?혵ÿk?"¼­4¤yö?|y ܉|?j÷ë>þùq?±r¾©þÅ?"B¢¤j¨á?ë(çÿ?¿¨Â?"¤M$ºu?{Kù8~1?¾Ý¹ߑi?œ
ŽÊ¡14FGL J0332.1-1123¿îJ¨hЊ-ÀH–s-õÑÀ:Õѧ' ÖÀ<lšu%F@¢Ä—ôþÅ@´L{՝?Õ%
¦w?؆B#æäü?þÚ®½M$@Ž¬7+¿î9_^4i?à°ïÁÄ[¿á¾Jô°¿è¸uAË|¿ïþ0Q×c)?ïÎ0Ö¯ÐAGNfsrq2FGL J0332.5-11181RXS J033223.2-111938?ïµ\áÌË?{ͽ¦Q&?QÀ"Ï'ð ?P#4´â?€€VM§Ïw?z'm¶@Ëë?ﺩ"N}?¡Ê¦¸Ig?g*¸öó\ª?~Êgï7¦?œCS®—ÄË?Ÿ7>zpHk?ìˆÒ"›µ¼?ž†¾Wþ¾—?¡ß½~!?¥ÃeÍ?²ÉŒŒcA—?–ͨm'U?ï/UÙÆû??"ª	ÑØ[?YG—&ÆU'?M©iºì¡ˆ?˜€ËT´2Ñ?"ZHÛËCd4FGL J0332.8+1557?íËu¥¯¸¦À?È)ˆ;£À;H™Ì¢ÛÀ<ŒÎóº1@ fWÎ.å?úàSý®(?ØÞG ÏÄ?âc¶ˆ½©C@ úÄV܆@ü0à¿íèÐ~]($?ïÙQu=™¿?…Ñe¹¿Ö—¼Ô¬j¿è¦¸f
{¿ïü¬ÄÉ%AGNbcuGB6 J0332+1556?ïŒÆæ¹à,?ˆÁ}ԇ?w-
ê,Ϟ?w|ßÅ7&é?7¿\q0?Œ¯å­%?î~;¥?¦$øP´•Ž?tEÖàdÕ?'Ÿà¶´Iv?¥"	¬!Ì?£ßËH–>?줄àåGÔ?¡ñ«u©v?˜JÓæ«g\?‰ëÌZïD?´É#ÿ*çŠ?›?í–t0?ì˽	ÍKþ?£$!Õhw?Šˆ‡î,Þ?…!ù˜§:?¶QÏ÷Úr?¢iÅöÔ—4FGL J0333.1+8227¿éðXBƒ«@5IPüqÖÀ:ÀAFmDÀ<¬Š‰[]õ@™Têèí?þC:sÆ?Æï¡
+b?Ëyˆ'!@®ŸÀ@.وœò¿îºadw?ïù·a*½C¿ä<Í`pƒ ¿×H¢L@¿â¦wÎm·¿ïㄟ6'AGNbcu1RXS J033208.6+822654?ïYù‹?~Íç…<hú?pŠþÁI?l(y°ÂÚ?ƒã¼|?¼"?xT@¤ŽB?ï?'³¬¬+?"Vóü‡ßV?l'?¥!Œ±?}¼ü[ª?"ˆá•ÆHÌ?ŽË9–ƒ#?íø3Ì÷OØ?'òÉ×c²?†#2ücõ?xÖsèÿí&?ªözcËék?
»ï¹P?íÑ«F˜°?éóƒ¥+?"Ó×ïàT?˜tX"XZ?¨¤a³>"Û?Šf>™x4FGL J0333.3+0233?ïóàî²ÀD~~¡ÆÀ;a .QÀ<‰<
ÍH@ GRBBÖ?ú{R¡ƒâ?ÒÁÐÅTÞT?Ôø'Äj'¼@Œðs›O@¨¾vÁ¿ïþÃÎ!a?ïò¦Ey†Õ¿áËZ§ƒ¿¾p¢ÕWŠÖ¿ëÁšÀ«¿ÕÝC<•²"AGNbcu3FGL J0333.6+0233NVSS J033321+023110?𧻓²Rð±?'š_í[ó?YðF¢CK@?WN×o÷JÐ?Ü
–ûj?Š´Ãˆ?ïh¢¡mi?'°{°j÷×?KÎÌHÊ%¾?a2<~¥Ñ?'
5zò?'…hPëE€?ìƒ&ÄÇÉ? ÌÁ'}?S,Uyo?6 Éu£?´'þ¹lY3?š'ÿjµi?îÊ¡@\F?…ݪ£é±Å?n¼0˜:òy?dñ,"X?¡j(ðºìk?"헝ý>ÿ4FGL J0333.7+7851?Ɲˆ
>â@2vF¿2/À9ƙWTz¬À<f£ÝÀ:@Ôµ'"™€@ÐÞªDã?³PSÕj*@?¯Cûq??øùìU(P@æ ‡4U¿àQž®+w¿Û˜0bôA¿â Ð$p!Ñ¿ÜOþ$ކ´¿á‡_<ü`¿è´À}‰AGNbll3FGL J0333.4+7853WN B0326.7+7840?ïLíy¦tQ?'0ˆˆ
?em»GVÑ?U±íκt;?"´™i¨‹?y'삇?ïqÁ+ñ¡¤?9YAeß@?]¬!Rú?lˆ'ì?îßólÀ?‹œ(Rl?î"ݽÖ?'í¸l½g?WÃÓ?pG¼ú?«Lڟ³ê0?àø ÝÂU?î;‹µY?†`H©º}?Ž#8ä®®?q¤y÷%Åx? ŒÓy~ã?ƒ.#±K"34FGL J0333.7+2916¿îþü°üHÀ5êÝYÀ9óæí	ƒÀ;­	¾º@U‹DÂ&×?ýV‹@š?­[åÂâØ?¸Ñ|ŸbÜC@‰Oâ–b­@—Ñ)(¿Æ­þÖ_G¹?àµbîᶿޛ¤¡4˜Ž¿Ø?"Š¾µ¿äg8ô=T¿â;ÊYêWAGNbll3FGL J0333.6+2916TXS 0330+291?ï‡}˜¢*?"û)æ'd‡?ZÚ4É
ãË?TëSüÅêÄ?ŠÅS>:y
?ƒŸ?ó"y?ï¼–6|ñ?š­3W?pÁ
^¼æ^?{«´H¯?™X)á(B?—¢Žd'?î*6H{a+?—ANyؼ"?4P…YH?}+L³¦Î?©‡s¨–ú?"…šuGÑ?êêÆŠ ¤?¡»poöž?—+MìÒ?~6Êý?ݬ?ÁaBkí¿Ø?¡ž	‰õ9¬4FGL J0333.8+4007¿î"®åÓ{_À)Á%µ¿jÀ:žjÇ7#À<^/",z²@ÅûÍ@@yƒœS?ƃuÀÌcp?ÂK´^kñ?úOfÛl7@…íë*†¿ïôäxºüÁ?ïû+‰>¿â: D®…º¿à¸‰9˜¨¿æX'r0t¿åPJ9ßöAGNbcu3FGL J0333.4+4003B3 0330+399?ï"uJ@i?€:hLÀ?T° S~'?Mï­ñ/W?ˆŒ«£U°?>Ž˜E«?ïV–0:Š<?uS€ª;?LS¦2ےŸ?`vt?"JœÇÛú?dëv6?î$…`3Õ[?ïd‰´i±?uk#·ë¿?d£9Æ 	"?«
E…Å2W?Š gaì?íÖ܁
?TŠ¢Ã™Ý?ƒ§2ƒß^w?möjN.é?­¨kM†wÄ?Œ`."¡Ô—4FGL J0333.9+6537?ììåcœ‡‹@^ ƒxÆÀ8üƒýP"WÀ;×ÛIgR@ \@LÌ6z?þ°®‰ç?­9Cm"x?¯j*$@Á@y¸_~@°E
%W}?ìêKBž‹¿Ç
A\Õ¿Ü*¸$õõ¿áÝÖ´¿Úr
žêff¿á!ðÐrAGNbll3FGL J0333.9+6538TXS 0329+654?ïZúWàç.?Žì|©¬£6?Ká&ê?HûQß?"Çýûb‰9?Ž#™ÃâÞ?ísÄ@Žò?µ¬I{¦Ä?]NÏÛd?t'¢3òÏ?³íhÀP'Û?µoÀŒ<ç·?팈¦à89?˜	HʘÍ?z÷ÔÇl½š?qÁW&.5?±ì=|‡r\?–fÅAÇ7?îÛîÑñ³?…4ýVO®?wO6˜Šá'?e5Á–§å?ž®X6¿Y?"µ/ÿkþè4FGL J0334.2-3725?Å©öš6Þ ÀK1–¦ ZÀ8V(LýàÀ;ŠÓ8÷˜R@vz†.?þ§]§{¬?¡$Xyé¥ö?±gýí<j@«BE@i¶ÉŒ&¿Ül—B|Q_¿Ù}Ã@1¿à_ÿ¯x(0¿àªjl…dX¿ãÑ}ÁKå1¿àŸì.'ãÃAGNbll3FGL J0334.3-3726PMN J0334-3725?ï¬Þò&ÓÆ?–Zp	ý?3	ÉÆT(ò??+q3B¾›?"/õ(m"?%Ða…'Ò?ï­¼'Tã?ˆ.'[ےô?<Ôk@P3²?M'Pi†|?ƒªV¨E‹?‡w¼•ÌÑà?ï	4ó³
p?‹ÈÜbÏ3?u<Nc5Ò5?qcöo-?™ŠMðÑ=Ž?ˆæŒöXN×?Òj{'?v¼¤û£¢¨?I˜h¨¾o-?9ú–­°bT?‹ÆDÚÕ4…?v€¨ž~4FGL J0334.2-4008?îÑÜߝ§ÀK	ˆ MÀ81"+sKQÀ;¶½-˜½@'Y‹b@žý¼XáC?—‡>¸…:?²'T>×½R@œ
²p*5@µ‰ÐMà´¿È÷Œ¾ê¶î¿ÜãÝ Á¿ã"õ¦n"¿âáÑa*<¿æà¹(«¿è à¨-±AGNbll3FGL J0334.3-4008PKS 0332-403?ïÞd9ä؄?sÞ#3±
?6ƒ]­0[Å?7'M"z,?nËZeqÖ?r²	Ý?ï»\íØz?f'ò)'?>ütñùø?^>ILUÎ?€0àâQŒn?€d?M-e
?ïWKÑU¦?'"áUïX?qát#Ú(×?q‰Í‡ë?ž(ÔÞÁ/?}bPÿù¿?ïôúzND?D¶.ÎÂ?!›õ¡)õ?Z×ü¬P¡?S׍oSM?C™3aN.Ý4FGL J0334.3+3920¿ï	yHkS¶À*æèÑQ­À:½lŸe‹uÀ<rüp(‡@!"nPj¦'?ý1?Þ<`Ù?¾%vkí¿"7"îfÐ?Ö¨"s¿ë=@3ÈÂüê¿ï¹¾GMò?î÷L!ìŽß¿âZr¦æ‰¿ÑuºÆ"$¿å˜<8d?¥y@ޗz†AGNrdg3FGL J0334.2+39154C +39.12?ïⓤÕþö?eTtà'î?1æÅpyð?+eÉÐ/?k/'{íZÌ?d<?<ÿsð?ïZ>QËDÒ?¢·=ðêbû?@&³v¨?^r'Xß*Ñ?"7àû°j?¢ 1p•®?îw"œxR?'=ËÄ0÷¢?q=JµÎ	#?[gyÁ¡Å?­ ä~¹À?'–ké0m»?íØÊþõ•™?"<ŽÒxÒ?zˆ'&y™?kÄyÚÝz?¯"=Ë×sT?"O•™ghÐ4FGL J0335.1-4459?Èü‹äÀGÀJwŽ}ܤ±À:¹é›9­À<z	d,ÐC@¼ ý¦‰l?ÿ¸ŸõÔ-?±êUéŸì¿R 	äôû"?œ,=mO@û5ëÊ?ïë}[‹¿Ìi"ïî¿âç&J¤‡¿à`ÃY†"¿Õ:5ÛÚð¿Þ`¸vÔsAGNbll3FGL J0335.3-4459SUMSS J033513-445939?ïè̒åH?i§·9i^d?+µŠGß?%‹77u݄?exv:'?h© Bۇ?ïØôTù|X?yv<NªsU?¹ùñ°í¾?2D¥$ƒ9?sí›{S?xÖ®6É-=?ïŸ7ýT?ƒÐ8¶®Ø?c†o#'ñ?[Ó9åŒé?œë^4?'óoÁ҅?ï։J#õ(?Z¢¸Û¢Û?6äÚ5Új'?&2‰ÅÇz?sM
J§Äö?YÈFjëžh4FGL J0336.4+3224¿ÐÄfñ?Œ¢À2²býüÁÀ9èT菡À;ƒT¦Ë±@ÓÝ@ß'T·?¼éÝú'Ï?ÞV›Ã'@Õ¸ÜU
@¥Í¸Úýg¿¸ó3hãi¿â1®~-,‰¿ë²¶°*Ö¿ïîªm&t?ꋪ=UËä¿ïïë L'(AGNfsrq3FGL J0336.5+3210NRAO 140?혯SRç?¹EËmA]?²‡Y?Ø?¸ÉÑ!×ú/?cŸÁ…=š?rˆ}﯎Œ?ëM~ödL?Ëb«o·ª?³ìÊïÍߓ?Çuúû°¹7?°É~þ?²ô_u¸?âÇ«VØð‡?´ìûyN?În‡YeÚë?± +WˆÂ?ÆrËK6b÷?©8ºüa>?ëQ¹'ù?¶]»õµÙ?—˜Å±ÔÖ? ¯-@zBÀ?À› cÓéˆ?³ú&÷+4FGL J0336.5-0348?ØñÅÌõ´ÀF—ædNÀ;Eag°À<JFu/W@"pø¶4¯à?ùìl5ç?ÉmŒàΌk?ˆÊ‰¦‡hÀ?ÁE‡ô€›?ÿ¥,ŒûÑr?ïþ¹^Zÿ*¿î' ×?ªqDC"l¿¿ÛfwBוÿ¿ÜTÙv({?»±Æ¡‡GAGNbll1RXS J033623.3-034727?îÞmŠô'?Ÿ7Ś­eà??°À)%š?8ðW¦^8'?¡ÙÅÐlÊ¥?žø`mƒ­?ï!hø"?Ÿ`þ­-5Ÿ?T³ãpæWî?i2,‹œÚx?šÐ"©ïª?ž'ˆcàsŽ?튘Yáߦ?•À$9
Ø?kWî"'*?Z$#«v´?²Ð}Àoî8?•IÐaLÏ?ê҆.b?¨,G­)I!?e‰x;ÈΠ?]÷ëXŸ¤í?Ä_ÁÒX<?¨HLýHä4FGL J0336.8-3612?粬ÃrÀJ÷¦a(9À:DՑ—l™À<m?æŸÜª@ȋä¥0§@[Ò#Mââ?½":'x5?—³HG8ñ?Õ螄ºåD@<¶a{p?1‹"G¿æèG]ÿ¿æ¨Š'¾Ú¿ëpê7.j¿ïøp¿…¼m¿ï÷¹_‡¤úAGNfsrq3FGL J0336.9-3622PKS 0335-364?ïåÑ{×¥?mkeðRÖ?So§é&?PSð'¢?`vöœ†ø
?iPí[˜§?Êc°?œÞgŒ=JÛ?iWIå)`g?{Íítš2?šÁcª^?˜N3$$m·?íš91o'‰?˜°ÓJ†AØ?Œ7ñ¡Â?ƒE^ÊDÅ?¯N¥ì£nï?"l6ÜÈUz?ï_œÓ?…Ù¶­±Çâ?Œe˜þE\
?€ƒ±ñƒ‡Ó?'ªç É·Í?y— üùÉ4FGL J0337.8-1157?ߪfï*ù1ÀH
A1"¸À:ž¼Õ,À<_‡ÚTtÌ@,³‹™Q@ž/Egé?ÄaJȦ?§ß"\BÃk?á"Ì`it@Ðú'­Â?î@aNÏpì¿êÈ@Á;I,¿äD³zì¿é¨aé)#æ¿â¨:{üС¿ïø¡œZAGNfsrqPKS 0335-122?ï7ØSŠ?–A¼ñ
q?^‹Ž°"?RˏlªîU?—?L7*¬?•È+Wåµn?ï¦HzÐ?š³Å•~?Y¶™¦
Ÿ?lׁw?›ÏÍ"¥h?˜.5L¿š?í€o°Š»ù?–Í΢Ð[?"QGµì?rM_ÏMØ?±rY›Éw?•3žÅ·?ï-¹¨Šrö?YÚ['ü?lv¸Õ{R?^~}ª@ n?–¹óÔ6ÿ?}<óÏ6S4FGL J0338.1-2443?àñ/OgÀJNœË}AtÀ;r–ÇWBÀ<¼œe%ô†@!óx"9®"?ûp)þ×?ÉÁ`ÝæO«?©Ü½ýôY{?äáý€É¾û@w{	
À£¿ïÜT\È?ïŒD±à¸<¿ÞaÁæê°¿ãáÍzq¶&¿æð莐§?ã笁Ӫ7AGNbll3FGL J0338.1-24432E 0336.0-2453?ï¯|ö°NQ?ˆ°ß&ý"«?8÷h'¦ó?4âû"š—Ñ?ƒY¯;u?ˆšFš:d?ïYÛ®™Mû?'mΦ8)?PKZñ.±´?`xÀ¸ñ¬?"¿Ô}ÃUU?'<°ˆ§?î
¤'_?'@0¼£?vˆ*¿x ?lŸçMš Û?¬Žr' Š?õŸ$uê\?í}¨š5b¦? Ÿiÿü(Ð?n¾áÂÐ?i»€ëÓüÃ?³ʗL\¹? ÚÿT\¼»4FGL J0338.5+1302¿æZóStFNÀ@w¼Â"çÀ8ÖÛjËÀ;~$–¸=Ê@ K	óô®é?ø"ËßgD?±2jáJ]?Å,Àþ7~@ßZ',•Š@=ZÿU
¿ïÿæj,Ą?ïÿô¬å¦¸¿Ô5Wû"‹h¿ÆÍ7€ÊÀ®¿ßaŽû°åæ¿ÜB"dXðAGNbll3FGL J0338.5+1303RX J0338.4+1302?ïÛÖÛo?'PúÚ^â•?S'€Õ…¬6?Y®\䃍;?k.éxaº‹?§rL.Ε?ïªb·då?žæÜ~=f?`i]¿ÍM;?j¦Š"f¹?›=‡ñ¹Ï?qüø¨›©?ìcÌk‡R?¦dág3?£'7;"DD?˜hãƒQ¬?³N6«E? ôÐøÓ°ð?ëA2Ý á?© UÍZg?'.žòՉa?rB°Æ'?ÁØJšR+ä?©̐sn#4FGL J0338.7-5706?ïÿNéÆOÀGþ+@öjUÀ;ø|·
èÀ=,:ñn@"ANoÑI?úç5ï¦?ËîÂÖSß%?–ï(lZÇ!?Í ÓŠ+<š@.Õ>5p¿ïî4[Q_n¿äùp~î©?ïþ$'ýu¿ÓÄ­ÄsâÑ¿êýOa<é?à@¿ºAGNbcu1RXS J033832.0-570449?ïÉ¢`7º?™¿M®\™Î?+Á÷R\›i?.bAhٜ—?z"Q=ü?™´˜ššÏ¼?ïz:Ñ I¥?Ý"/«v?A£ÍeŒ¸?VóE‡)"÷?+‡pÊkO?.Ú7U?íár§—	û?•âä"Oq?CŸ.û'?€Š´´ç¯R?­—í¿C¡u?"}(Ð=7?ï#²auÔ?‡v…ƒóÏ?Kqøz·£?L¤ÿ½ê?š®+Q™oÇ?‡Nv˜ªá4FGL J0338.9-2848?ê#m­Nú†ÀJ"K±¯:À:ŒAœƒÀ<^.bT@&n¿%oP?ÿ…1˜(€R?²#M"M2¿—Ÿ'ya7J?èrŸæ¿@àP64?ÁH½Þó@¿âXœ‰8#¿â@^"àÍ5¿ß	Ñeõ¿Ü&D!íæx¿ÆD
›åNNAGNbcuNVSS J033859-284619?ïß|M""ù?e'Åêå'Á?7G(íX?0ôÑjÊÙp?mš¾ÆNe>?d vÚ§s?ïÕWJ'ê?{sH]q7Â?/&-S?7"®Q¿ó?t۞Ÿ6ƒ?z̒bp?ï=bF?{bM©*ˆi?`ÒV(…_O?Hfܬ¨¥?–9lw,Sw?z[.›¯»?ïÆ¥9ç?aQ0nè†Ï?6_ÈJ6=I?(?­ 0R?{(¿©%?`û	Š…À4FGL J0339.2-1736?çћ̂W¼ÀIG"#ÐÀ9•²F8ÉuÀ<\ªûÁ­@†rK!œ?þd¨Uôÿ?°ÍÂkØ?¡ØÎbÏ1?ó'
8ͦç@w|üTú®?ëpø@¿Ð‰§»§¶¿áC™b<5:¿Ø´Ó[Ý '¿àÇ7—FC¿Ý6¤!1þÖAGNbll3FGL J0339.2-1738PKS 0336-177?ïÃ×-'Ž ?rwsõN?EzŬ€{O?9ÍÂZôñ?{e( ,?q'ANŠî?ï°Ö¨ñd¦?†ÈºEC˜Á?6àeÙPP?K|+0?ƒR–¸å?…À\Aş?ï,ëAé?"uçõ+?hõ¹¡¢?W÷5ž±q?œècô+™Ï?ƒ	!wš=?îü¢!B?דÀªä?lM¿ßë­[?WHÆYC˜ž?œó3¿ÚG…?}"Âï›ül4FGL J0339.5-0146?ì&ֆ½|€ÀE:h±šA_À7qëýê|
À;gKoj'@
Qg¦­S@ðÜá?'Ö•<VŒC?´Ý)¼<ë@kMHˆ/@EµªœK¿ËûŸú[Ñ¿àÍìlø¿å€…áÖÊ'¿åÒBW"¿èæWbg~>¿ç]™£ª""AGNfsrq3FGL J0339.5-0146PKS 0336-01?ï¬_ÿO©Z?t%ó?S=éW³ã?K²‡åNª?'€C,ã?s:ÛªTI;?ïr΃לÿ?"мe–Ê?Owͼšÿ?cDŒÀ§¡?ªqN{R?'þ:¾Ýèl?ïZț(4?'Yþõē?z#€SœV?uv¬¨Cy?Œ<O_Œ$þ?{¬fˆ–k0?ïï^štŃ?R—ÿ[ÛF?3fT.1?.ڍž-ÿ?\i6
貏?Q"•
—U$4FGL J0340.4-2422?Æ_ǦGQùÀJ ÝDÀ;ö,A§jÀ<»UãTÏ@ Oa<0?üz0bžZÉ?Ñú¦]Í;?Ù9Ã¬è@$ž¶,?ú©W³è¿ï×+Ë_åC?D8>5?łZ7Ùá¿Ö~œÚñÔ¿é5­@ÀdŠ¿ïúö`™ó²AGNfsrq3FGL J0340.4-2423NVSS J034022-242411?ï6@è³3g?ª#fž?}°ò¯q?x톲Q/¨?'ËàìíÒ3?‹¢e5?ì‹q
@œÂ?¶V!?˜%5Dÿ?¢"÷Ú?µ›*U)Ú?±™®	2'?ì,4žèÝ? çoŠ1P`?¡öCÛ?'ŸÙ"û1?µÞÍ
~¯?˜Õ°QlÄS?ê¿Àö5˜«?£TLì¾þ?¦*wb…?"Œ9&+¢
?¾ì¼ÆƉd? ©ƒa)Ëp4FGL J0340.5-2118?ï¢Òj›MÀI–Ñ¿zÔ²À9E?']<À<Ciô`@©÷è‰ø@Á°9ï?ªî^å5?°0Y9(Á@'ÿœ,ñÑ@
Ê*uõO£¿¤øÜc˜¬¿à@úœðž¿äÿT¿:¿åqøÀƄ3¿à]s]Å­õ¿è ;tJT¸AGNbll3FGL J0340.5-2119PKS 0338-214?ﳺ]ìâE?}rž.ñ?;±…ãïíG?3¶Yõ¿ï?'3ÜU§ïW?|Þ¯ŒrHf?ﲫ"UÑ?"ëÖIÍø?5X+u"?Jù\×
í?'ÓÜ)0	?" ؼL¾Ž?ï->ÒQr?€¯¬õˆ?j`9Á?\Õr‹É?—•Û¹'?~õmwD?ïÈ;x4K	?dy®šÍ'?XÞ½‰©\?JvcŽo}h?uª"ƒp#Ð?a3ùYÎL¹4FGL J0340.5-0256?áLèvª	ÀEtžý†¨üÀ:ªÏmýÀ<Ybцoñ@'{^p"Ó?ÿøŽ‡à?ˏhc?Ñã<$ôV)?ý
O#SÂ?ÿ‹çýÈ?ïõøÀ·¼¿ãí¥Ùÿ¸…äÛâ>y¿çƒ¿ÝÑ¿å(R. ý¿ïÿA^o! AGNbcuTXS 0338-030?í½¢ÿoö?¤r{¬á´ü?{L傑G?r9LÒ#˜0?°bԏÛnÛ?£l*P
?íŠË¿õ0z?«æAk?Ñ?ƒ>±_Ô¤s?ˆbUÖ¶>?±AËÔ[ç¥?¨ë"?1šÏ?êä;7#ãÁ?£—þÆß?£ûÿ°õ™[?ŠF"õ\­?¾à&nfH?Ÿ«$fèÃÝ?è$áXM&|?¥Pì`Ó?šRšÓ* ?‡~nåÙë?ÌpKq¼?¤×Ab…Aç4FGL J0342.2+3858?Ä:™)ÃYÀ)˜øçÝÊKÀ:QÝIÒÄÀ<9à+Nbd@9ºZ.t³@üº€™îS?¾–y(µÖ¼?–Úâ}ýˌ?Õý†þâHµ@NžT¿J?íó
¾¯}²¿æ4M¯¶;'¿å¼ùðòF¿âˆ^Þ²¨¿âÞsV–¿ëšŽ ¿"(AGNfsrq3FGL J0342.2+3857GB6 J0342+3858?ïí›1ç}T?V'¿
§ii?0¸¬Óñ?%J÷¾uß3?`M¸~!,¿?Tp=Øú'a?ï±/î¯`?–*?rš$ð?#6"e¼1
?<6š0ížF?ƒg*B¥wc?–˜j/ž:?ï	]~¥K?'¼®{¾îÜ?i¯²aø—á?[ô›ñ·ôd?›žYߊÜ?
lMq^?ïɯ}Hd'?cDüÀh Q?1KÓÕý÷?![W"¡Ç?zLžŒi?c-ºÖÂÅ4FGL J0342.8-3007¿ÄõÑË0·ÐÀJ>U⊤3À;\ù1¯¥uÀ<è~ ïÏ0@|ØãÀ¯?øï»åüj?Ý儠¹?ãJB¾ìdm@ l‡י@Úën"d¿á²ý¸ýâï?ïÜ¢ÍõÁ¹¿Ô—€DY¿×Aß3ÞL¿ìŸ_¬8¿ïòÛßå-lAGNbcu3FGL J0342.6-3006PKS 0340-302?îSCGþ¼?¡XÏrj7?œ'"
Õîq?•
þòfö?™ptõX$?•éͼá¤?îQž•Ð2y?¦Š¥ðŽ¾?x ö»'?ŠÆæÕV?¦÷"%u¬?¢
P±Ã·?êñx´Cç?¤ô×úOu?­{|Ñ÷¾ß?–aĜ¿Ä+?¹¶{öÊX?{hán,Ç?íК,ë¡L?•T²"'?…ì­+vyÝ?Ñ.§?­{1æhLÖ?'Ð25¶4FGL J0343.2-2529?ên*æ±OÀIÓ|ÌyÀ9ÊdpÂà»À<d‰éù-~@Pm"½¿i@±oɼw?·*Aë1è?Âo'Ÿaµ@¡âއ	t@ҏe?Ô‰[l¿ä\¦(ô¿æ߆ôÛ	¿èq¼Û¾¿í2ê£whí¿ïüwIãxáAGNfsrq3FGL J0343.2-2534PKS 0341-256?ïâdò>©œ?bR¥±·º?V™ÁTbÁ?PËuuïŽ?bN`¬2S?\§EÂÑ9?ïÃÁ•Ç?Lÿÿ?:úÂì'#í?V¯páàp?|oŒ´)Ì?Rô0mšå?ï;³é³W£?»®+ZÄ?rgcâÆz ?hVá⹚?"ï©Ðãlâ?yëòâb¸?ïìOžL°?QÁ³'Ñ°?Au:}áR?4›ª]Œ²µ?^¦&ò§±#?N(ÀqĂ4FGL J0343.2-6444¿íÈBYÊTUÀEÔa¿7¸ÔÀ9y'S+ ?À<Sá,Ö"@ýt»¾³@	…º¿"?¬IƝˆ¼}?§áUšç!?û'YY7©º@Çl½Ãp?ï ±ád"¿È™òD€"¿äCN¾ÿږ¿à`)k3TÁ¿çí¸4Sſײßð–AGNbll3FGL J0343.3-6443PMN J0343-6442?ïâôæL&?dћË?'ξ™1¸? Ý÷Õœò?kŽÿ-ÊG3?dIñÙd[?ï¼Ý=ú߯?¥»è´5J?-WϏ(/?Cì
01p?€SR'	×Î?N;6qñ?ï
 q\7?…Rñ1¬UF?m`e)JPÝ?fºÃ´ç›?šÿå9k/?ƒ{ì~''F?ïÎÌʘ?a¢BɑŒn?Sc×µ9?C‹hù
?tˆÖ"Fñ?^Éd­˜44FGL J0343.4+3621?ì§þ4+‰NÀ-fãOÆñÀ9ð¿§J\EÀ<jÃQ#@®Uÿfþ@€W$'°?ĘvßE?ÃÕYä!þ?ý&¾æZ<Œ?ÿe*ß|¨¿Ð"á+~‰¿é¹vCS;ç¿ÖÄO»)6Z¿çqÿ Üï¿ç
J5®7¶¿ïëa½µ,ÈAGNfsrq3FGL J0343.3+3622OE 367?êÃf9Â/?µVÏprsÐ?ßèøƅ?‹"X›Ñº?Ã÷viùÞt?´!'Fo'Ê?î'LC£?¨
§–çs?€tTΠÇ?‰êYöt®k?ª2¥¶ ?¥à%øÕÓ?éJ'PÙ?§µÕ7>±?¥pòí"w?œ´ôP?ŐcDÿt?¤½Î"QíÖ?éÏ@³f¦?¢×l"½Ù?_"¹ÎŠ?…gG+˜?Å
)ø¡Ó?¡dB™4FGL J0344.2+3203c¿î¢­ËšÀ1ìP½‡µlÀ9q±6nQÀ;5º‹¨â@ÿúPh£-@qÅìÞ»?בÁŠúD?Ý×°UÁG@"˜Ã°ÄY?þÎõü›ò?陊€!"¿¿T³.@/¿è«ÆÑá	¿ë!jÃQ#¿á0–5a
Ý¿ïí%g˜•ŽAGNbcu1RXS J034418.2+3209030?×3§|Òo?Ã
é`¯¤?ѸôXšóÁ?ÄÒجó{?×üÿè9Î?Å°ÌrfB?ןÝ
%?Ò-"MñҒ?àFF4€?ÓÅ)lúçä?À¯,Ó!£µ?¹wÅBR?ÒÞ´&-?­=*Êß#?ÊÂßáŽí›?¬¹hl£?àDXýB1"?°È1E¬È?£ü«/§òx?Œvڎ÷?È?Óʯ)á¢?ÁÓXÕ¢-W?åOõp?Á›ÑÜ=14FGL J0344.4+3432¿Î&Vš°4À/ô‡B_À:ÿ@ÿ¤À<ï< @!v_[…6á?üÊÙþ
·y?ƎDÑÁ(T?ª‡1j…@?å‡q^-O@WDŽ¥J¿ïö«!ÃI?ì{Ϲçû?È6â?OÌ¿ÐÑLŽNý¿æ¼Áò~7>¿²PÂæ$AGNbcu1RXS J034424.5+343016?ïÃIbYEì?q7•×P¿'?3Ó S†?9hùîña¸?}¡WÑÆ?pä%8þ?ïŸyÙóá?Š†‡‰Q?9—c$lË?PŸø45'Ê?‡TΦ_§\?‰¢[ÙpÈÃ?î2À^¼—N?–Ò´4W¼?o1¦ã½ì)?]±n¿j!?ªàߥú¬l?Œ.þŒÏ®X?îK¡ž]i?‹E
—"Ø?pØÄù[?`â®w»Æ?©4ÍVýó?Šsiè"R 4FGL J0345.2-2353¿ÅÑc=ÄÀIj³=¯øÀ9@ßìdAÉÀ<Dªùš‹@ƒ°f·š@G÷`MÉ?ªÐÌ`Á5ë?²¿ïn¸D€@P<Íæ¨@	n£Rÿ•¿×˜ÑÞ«Ü¿â™ð‡Ôö¿ç¦]¨R¿åˆGä¿äÑTá®±.¿ïÿù_|è3AGNbll3FGL J0345.1-2353NVSS J034518-235218?ï³õÂÙéÛ? ^"¡ý?G·ÒZ'©?@´}MÈ1?‡#Û±? }y¹õ's?ïi˜Ä?¡¤€GFOƒ?a7­BÌL_?u•pU\ð?œK×UB¾'? ‡OnKïŽ?ï-ôjy,?e—ä;ûÈ?l'Dºy^?g¬ûô¶!?–¯J,y‹G?~j¤µ…s?ïX¹÷ët†?}pT,<i?~ÿŽ:c‰?k	mÑ`'Õ?ŠQºçñ?v2t8ÿ4FGL J0345.5-3301?ïD­. ûÀJeè'%À;(*FûgÀ<ÇMé—Þ®@åכ‡Û@lCõù?ÆÐ=…³:¿'ÈZ]É?Êá|œ³ªg?þ|jvìEŽ?ïÇ@f!¿è¢®Á¿ãq•+uпæ£Þ+™á¾¿ÙòÑäcÂG¿ïó²I"ÇÉAGNbcuPKS 0343-330?ïÁ˜ˆyÓ?…â¡\.¨?KOŒ-¡?Dޏõã?Šß$ìhÈP?…]ÝÐà€?ïU}Dó'?'µ)ÃM_?NêïÇ«?`qz+2?"Y¾©|º?¦0nYnš?ît͊±?Џ/#Î?|á웴Á?jy-¤J´8?ª¼')ÁxN?Š:D+ÛNG?ï(d?·§Õ?~Âæ5ì†?b"it!Ò?T]¼¬{'?˜¯*چáj?~®ùÅcÖ4FGL J0347.0+4844?똅â'Àg|¯Ý©À:tü+_)À;¥ðFN™@²Æo­G@©âå=?É?:èß'?Åu°†E)?ù´…xze!@Í~¦#?Ë?æm®YD>ô¿çnµŠè¿åK—"pî*¿ç—IBi1¿éöÒÅ4R¿ïþ YQUAGNfsrqIVS B0343+485?êPçä¨p?¸y0WXÔÉ?"óµ¿¿Ö?|
¡Ê'?Åu¡%bB?¸@€¦Ñ?ä2Îp h?ÆÞHemÁ¦?gðŒ}
³?zäƒ9Vò?כ¹J$ªõ?ÆÒOï?éY®øÑ<?ªÃ8{â?•µƒ¡ç‹h?''º—Û?ÇäÔÏßÉ¡?¨N«áà…?ë睆î?›çՕUˆ?†×*°—÷?jØ£:±?‡"JÚË?›‡l³‰ÏŸ4FGL J0347.7-3616?窅ZzþWÀIÞÿ´€¦À:Жï›-îÀ<¶¤À>I@ý"õ•Ä@"÷H¡Y?ÇàV
??¯¬3á?0Ô?á|tŤº@¼dkd}¿åÎÃ|Áò~¿áŽ®žä\6¿â÷®aÐ*¿å°B½ê±º¿ä•^Pp¿ïÿð ¼x—AGNbcuPKS 0346-364?ï:[4ê1¬?¸>±žÏ÷?`És?0Á?ˆYúÅ{?–¤ 4Qä\?µÚWÜ­ŽÐ?ïÙ²Žu¹ç?yCˆ]¯zÁ?êGÓæ?47:ç¨(?r¾I!í
?xšŽAŒ!?ï	{S›…P?'<!M^¨=?h
*öüaš?_Åù0{Õ$?›Îð-¯Éô?€ñ'/',>?ïö™È™ø|?>€+¢X…$?UT›Uj§>û¿æç êÔ?RÄ'4]V?>+Ã]ÃÄm4FGL J0348.2+6035?´³ Ž£@?Fí$[)À:""W:yÀ<H§+R""@!ú»+Ìw?øê`üšò?Ë!¼•?ÈIÕ·3‡?ö
ˆºNE?ü%1uBø"¿Õq7eGœ¿çåaHÌ"¿ë¡h?¯mk¿±"ùF¨Zý¿¾‹$ƒB¿ãēBgƒAGNbcu3FGL J0348.4+6039NVSS J034819+603509?ÔS¯•Í-?À|NDø?|•A%s¬ˆ?u!óÁÉ?幫¥ê2?À¡Û\r-?Úeÿd1<Ÿ?É`´ÆF4? `|e1Ü? ¢`ò¾,?âV~ËõÌè?Èü.'ÌÉc?æÌË&(?©X6¬¿Ra?"J=Ñ*þ°?}¹ð2h?Ñ1Åö¡AÅ?¨¥ðI´?æѝîg-?±'›ÅV§ ?†o®—e%Í?ƒ)»†D¨?Ó2ßOhv?±ÑÛ).4FGL J0348.5-2749¿µóª|jߝÀIv†œfÓtÀ8!ײÙÜÀ;¤ÖO,þ@ž4ge¿Í@³¯Yõ>Ü?™9Æö*?°(U3¹
@ÂܱF^‰@ qÛ	¦qï?ۜÞ]	¿Ý s]Dԛ¿ãÏwÁ¶™¿âOðِ¿çs4_Ù'¿ãUOwÅAGNfsrq3FGL J0348.6-2748PKS 0346-27?ï³";*á–?uûgü•û?A»•ž¿©h?7"­ŠS·0?'·Û[ŸÑ?u…ªÒâÎ?ïÏÐ.ë?~Lôܶ_°?-ÚÔÖø?JÙðÞvÔë?w)(ÁÒ¸0?|ñ=|&´^?ïB§žíA?ŒÜ*iú[?s"ûÓzrñ?rP,p෋?—6lC»$?ŠÊçf˜t?ïþ"`^ò|?ôa®·+>ÓÞ··#"€>ТG÷‰K?&+S+?À¯EF²4FGL J0348.6-1609?ïÿÌeÁbÀGÐqÞi­CÀ9˜®Eù•À<Lso"
@V0S.ü@¥M–Ãü?² Êzâõ-?¯²1k

?úÆ`¼Ù9Ã@…‹TÝR?ïÿµ¿â'ºí§7è¿æ¬êÿ½ºá¿åО~蝿Þ5xó0䤿ïÿãåîAGNbll3FGL J0348.7-1606PKS 0346-163?ïåC‹Ý¶ë?q"Ð΂F?*~vè³M?%Ÿ8xU½«?iŒ³ÇŠ¯?q2² ð?ï®÷8YŠ?‰¶
"-?:%r—ÌbJ?Rååûpz"?ƒqTá:ø?‡Fò¸ë­?ï
ý¡Q?…ØvU?póÜÀ±Œð?qp#OņÄ?še±'®?ƒ¥pF¨?ï´Kù?h0_€Y%d?`ýÚÎíÔ?Q¶Œê¹@?}wó…ê?dÖ>'r»4FGL J0348.8-0828¿ìŸ5Õ¿ÀFU•:À;ážëèòÀ<Œb¥Æ!@·ÉI	´4@Í6´ÇóI?̲fnžï¿qÁŒ/U‰?©}GÔUd@Ã3ºÂ‰'¿Ê¤©;¿ê'Âó/7%¿ÁüA""´…¿â=OG"=¿ë&Ü"U?x¿ïý—"ãwAGNbcuAT20G J034845-082422?ï0O#D"¬?–éWsnÍD?a:E­áÃ?Wok3¸1?—ÎÒΈü?–z:<½?ï-7k®Vß?–¢Žvãõ?Rgt$Ë?cmúؘ?™2š'ò×M?•
vIÐU?í©¨)'rÍ?"G«†VÞ?Ž"C@ø^?"ü/,M©?­Äl"Õ?)SÚ?î‹8¸'"è?ˆ²ØðB»?dè!O?V"W\«ù?¦Ã(eßd?ˆW^EÁ
4FGL J0348.8+4610?Ñxjfóv|À¨¬\ý
À:Œ|¦CÌÀ;ã¦êºô]@7Â4moð@SÍÝnÀ?Ü»"¿e=?çcÖ>»@
"x'@	õ¢š¿ß!Ã~ðK¿Üò{}Nà8¿é‹?äœw¿îÂˌZ춿ïΌŠ½]Ä¿ïÿþˆ0»ŠAGNbcuB3 0345+460?îÎ6ze?¥~,7	~?'ê‡RgÆW?šy6X49y?"N¶žK‡Ž?œL5›glÜ?ÑldOI²á?Èß´Ëe6Å?¸@²Ì6d"?ºïû-èº?äA·~ÔZ?ɕ²"ú£?å÷ç?!_?®éj´0e?»2åw(Íá?¢'µçf-˜?ʆðGæØ?ª!N?4t?ÙPÿûï€\?´w4‹Ç?LjV{€ÞF?·G²>4?ÚêÔÆP'?¾úP	Ä4FGL J0348.9-4859?îïڈC¨CÀHÌM©>êÀ;i%ö3ÎdÀ<Ù=x0"F@£Zì4Ç@«ôz¿Ö?ÁýHëC¿µ¡ÙÀ6wœ?óÙ¤ì³òá@6ìÕ*ê9?ïF®€žÐ¿âH†`Կꟴeͺ3¿ØÜ̉°îJ¿ï÷b|×Â?ïÖäH•AGNbcuPKS 0347-491?»E½?pNc"M??^,h—(Þ?k7Oe!?w'|'ê_?|«FÛp=?ï4Óéý?™IEý±?X~–´Î·?k6ÙQY‹
?—Ý™kÕž?—ÙBâM?íÌ[žÿ9­?•Nè¿n?"wÝ J?s÷îbZF!?®ñ¨¤RŒ?"=pÚ°>â?ï,Á¡¦½?…;Ãԁóø?p?ïd—m?dŸzÄÃG?–]ëòʂ‰?ƒ+t|É4FGL J0349.4-1159?äŒhv¿'•ÀFÚ$5inYÀ:E†ö(æ©À<R°«#@ öODú?úUPÊï$?Ãþ>ß¹¹u?°'_~ØÕ?ìRjÑ/2@8®©K=k?Ÿd³dÆÔ¿ç\ðû¿åü½€S¢?ÈS™Z.Ÿ¦¿àuïÛŎ¿ÜìCŠ™AGNbll3FGL J0349.2-11581ES 0347-121?ïLÍv	O?'¢5tq¢Ó?QÒá"ÏSV?C 7'™Ôc?žÙ88á?'fëQÚHY?﫼Gw/¤?"Š¹Ñ,e?2Á3å?Ag|?"€Õ<*w½?"¬("%p?í jOH?š1~pƒ?xC¾»'?gÊ¢T?µx|˓b?˜ûf.£|?îŽ}m4p?ˆäˆdF‡j?ZwVQ¯2#?Pi>»ÿOB?¢ÐmvŸ?‹?ˆ"ý8qóÏ4FGL J0349.6+2410¿ëÜbTf'9À7°³''dÀ:·ÔÌuŽøÀ<8.Ýc@°ŸÑ—ö@Þê· ?ÒBh$¬‡³?ÜV܅§tN@KŒ@Ã@	ޖMß²¿äïÍug‹¿ÞÓ0~¢ó5¿ëÙúnƇ¿æ‰Éb4'¥¿ð?ïÿæj,ĄAGNbcuTXS 0346+241?ïÏÁýNçÏ?~ÓÔØ!C	?oú©b#8?u<Q¥ò?`CYNôø€?ib\§E™¨?췝yáü?¸ö)šêgÌ?øµIXz?«Qé~N	?²ÈÝÁɚ?±EªýÒ]µ?ì©ô9J'?ž\‰vTW'?ŸG$î1'?Žq!Ám»R?²åw"©dë?–®›"äÉ?ì
ÖçÉ3µ?¥òo:F´?–eE=Mò?…é}øð@ž?º÷rvNÖ?¤#²#Òd¸4FGL J0349.8-2103?æØ£÷…KôÀH"tûTŸ•À9€'،À<·ÀÌ
Š@ÐÃAØ@¶øº'`æ?«Û®¢Ñ?ƪ[É)*@Aél?Ä;@w¢jxš?ºËŐÃ\6¿âûMÿm'¿æÊé½ôAÜ¿èÂ:ØC""¿ìd3áƒé¿ïü³µ¥iAGNfsrq3FGL J0349.9-2102PKS 0347-211?îÔ«@ø>?œS	¥+d?—Ü •¼?–˕?‹û%€Å?‰þ\ôO?õœ=3?6Rœs•?MÇ«lÿ'ý?^fђ—c?Œt‡â »M?Ž¨Õ22?íhÙÄō?£²"¦^ŒP?Ÿ0"+ƒí?•'+qŽÄŸ?¨!ÚRå"?žÝÄ:Nê?ïÙ2žó×Ø?`tqÞA¼©?U ïíG?J"Q$?kü遱"J?Z
®Õv.B4FGL J0350.0+0640?éIèº0ÀA"ãÞaIÇÀ;…BêÊÀ<–'nQí3@#Ç£Œa¢²?ùN"wÉe9?ΝñµaÌ?aoyyWsž?ž]÷íÛÕ?ý—ÁREG¿îb,°b2û¿*Ù>ís¿éTr]•‡f¿Ð$÷0M¦¿ÕÝìd—¯4?Á].Cà)¡AGNbcuNVSS J034957+064126?ï¶<B)˜?|«K'ª‹?&§ÂÞ¾J?"Õf'†Æ?'PjB!¬?|b`øº]Â?§Ši?«vÕô_"?[Mnz·è?nß÷7ãwö?£\{곪?«)pø¢?í¦_,?gå?šLΙãJ?j@Á9;o¢?WúhúÕ³?±û":åV?š¥®q?è[Êúü'?ºÓ9ñi{?p€;f‰‰u?sŽêTN§?Ï2ŽøßÁq?º\¬è"//4FGL J0350.4-5144¿á=B‹j׺ÀHDââ¸Ç\À;ªœ÷,À<Ç÷øʂ@ Éh»€I<?üªzýÍÙ?Ã:h[´×?ªà#Á¦(?èÛB±Ux@žÞýÑÒp¿îÔ;kç?àÖD°39¿ã&…¥ÆΆ¿Ð¦c"¥¿Ü¤ßÈÒí¿Ú'Z›WûAGNbcu1RXS J035037.0-514457?ïÆü\` µ?lr>?7èÁê'?.°¬ùÚ
?{PÃÑ?k[l'@  ?ïªGî›<?"4mXÞT?1äÜn¤ï ?G
¼ËÏá~?"ÞÝu«	Î?ƒŠNÒs?îa"Xn°?ŠaCf°µ2?m'Yé?Y¡Ö…Ÿ?¨
¨º
ƒO?‰:&Pc1
?ï9À'ºy?{1êr…5?X±\ù—A?K$àP:ðc?—<×ùkÓ?z¾uëSoz4FGL J0350.6-3226?êìî‡K}ÀI"ìé¢ÆiÀ;ØÚø»À<ÆEéïƒ@½Õ
8!Ú@ÀRP.ì}?ÑHµüPÈð?Ï¢$Ø|ƒ?ö!‹»Š…*@3I!ßÏ?ï­¾Ña‡¿Ø؄{zIÈ¿ã<6¢(‰a¿å
pᔅ¿çב#'¿ðAGNbcuPKS 0348-326?î"ÂT??»ûî¦ö«?wuؘÄê?' ›TµOž?¤Å=ߨöç?¸[`sãñ ?ïȘ»+Z?€Û€»¸öÿ?%k´›U~g?@©#vJÊ?{DÅxI×?€Z[f	=?îX½›Žø?',I Í‡À?"7B'6Pa?zL§‰'?¥fU¢Ò[?Œ§²!†?ïè0ÆO?S «–¢[?"U$=¢í?Ëe¹Ãd?f©ço_!Ç?Rà/U@¶4FGL J0350.8-2814?äŽYW'Á—ÀI@Ü­¡À;;y‹YÀ<¤v¾£>^@"ÒB?úkKøüր?Ëv5{âÏn?¨g=beø?ßUŽ7ï@;­$æ¿<¿ïÿm¾Ÿb†?î½µ7"Ñ‹?É®«d_1¿èÀO`c?Ñt¬¥:¿¿ãÎ#¯1±SAGNbll3FGL J0351.0-2816GALEXASC J035051.31-281633.0?ï {¢Í¥?~Š X/0æ?5}NÿU¨·?.sÐ	»>&?}Wí>£ÓA?~…Ä
 ?—ÅcR?Šjöò?8 Vô©\?NƉs]?ˆ•5ï†#?‰-Äruس?íÝ7ݛlÑ?'Ä+ÕÔ›?w:Q쨶?nòÏò?'ˆ?¯E8˝Ý?Çàc(ìç?îÏ9(.x˜?'rqH‰lC??ÿ±eW?B[qݘfF?¢Î3}¶G­?'t5 
Ú4FGL J0352.0-2516?âõ·^wÀHÕ³co;!À;R>{fÀ<Å憲6I@}pŠìÙ@"Pi¤ßH?Ó°°!á?·óÔMŸ›?䦸ÁRT@fA'šÇ—?âd"¿éöñL¿çÛBEÈa¿Ïˆâ|·`ª¿èàYTÔ¿ïúÅÞÆõGAGNbcuTXS 0350-253?ïí¿æ^ƒ?BœµK@?X§ÂãX(?PqŠ$—Â?ˆÂ{ô@?€­³Ú²b?ïHk³qq?'1SP»(F?N
›Ëa¯;?Yƒ÷؈ø…?–³'ä€?{·ª¤[?î!ÍÿÄöV?‹K'JVÈ?zFÔ¤*¹?iϯÝo¨P?ªšEo+X¦?ˆ$ü"¿?îô:^=I?ƒÛßf2_T?eX^D#?Wñw­1h?žÍ¢,–óÄ?ƒqbw‰æ|4FGL J0352.9-3623?ê¼3Ô\§åÀIYJôðØEÀ:øº˜â›À<uä;~[P@!@iGA]?ôÜZ>9÷s?Ê^Í?äF'?Ó7þ(Š@	™N?Fg@µt«ùm•¿í·4µs¿ë¼=¾&–Ã?æC¼ª R¿Õ‰Ïa§Ñ¿³`#%¿âh'Ü\AGNbll3FGL J0353.0-3622XRS J0353-3623?íúÒ÷ø‰?²Ýù0•×ù?{7ÉÍSw?x—˜(àD?¬ë×lfÍ?²YcÔÓ?ï6욼Á¸?£Õ%Cýi?N±:ì)MJ?_)¿H¥ü?˜,âÑ~Ÿ?£ŸNÝÚkL?ëÝsd"BÊ?£Q®S&é?–*å÷7Õ?‰žÞ*äô?»"!è¸? Ú²ÇU ?ìúÀº|?¤
ÔoS²?C`M‰·A?DœéÎYì?¸–Öè(´?¤Ö@Óú©4FGL J0353.0+5654?Ï0竗ÀH@¸ÌŸóPÀ:ÚH¶RÀ<VÅßrÂ@ jÞ~¥øM@CÂb¿'?ÀŸR–$ïù?µ´"K æ?ó5'éSì@ŒS'Þí¿ëo>&VV?ïå…?ðZñ¿Ø½ây1o¿ß,'Ûç¿ä'è̱¿ä61_žv"AGNbll3FGL J0352.9+5655GB6 J0353+5654?ï—îÉ:+ø?{â•ÐR®É?I~Ou.?@šÇ;»Å?ˆrŒ™
™?{&¥\»?íL¥üéNý?·çÒWÈ<
?U/—ç%,O?q(²æÙ?µF¹óc?·v
þ÷àû?íø¸‰Ä…?›3o(q´g?}ö°öp'ö?mŠ¾/zÒ?µ˜Ï,JÒ¾?™ªoÀ<Xœ?îÑj<q£‡?êØ7u'J?rQg}ÕO?]iӏ`•ù? Ÿ/I+'0?°Go¿4FGL J0353.0-6831?ïôáªÅÀDbŒL˜_À:r)ñkÀ<qä"rÁ@!ñnmpñ°?ú.kßL+?¾n­¡},•?›¹·Ç,#õ?àáP¢"ϳ@ó͞Xñ?ïT{昿Ú{´Á¾%ë¿â'OÐø«x¿ÑĪ¿[Ë¿Øše¼Tº?•©˜5ÁXAGNbll3FGL J0353.0-6831PKS 0352-686?ïpN—Ïõ¦?Šµ€0Œ4?Hlé¯Øtî?D‡ø¾W{ß?'2Ÿ'‡µ?‰û"×^…B?ï@¿}¡?"qƒ€Œ©h?N	×ϕl
?Y
òêåʐ?—
¹_³ …?' ®¿BÐ?íf@a"N?™ræh°²?vw5Ü{Ûu?l¦è5P…|?³fŒ+ŸÔ?˜õÃÕa²4?ì˜æÜÍF†?ž Ôú»%¶?}(KæMs?p»Ù È?¹fD[5ú?ž-)24FGL J0353.7+8257¿ìÈ@">Á@6Q?´‰À;X®í¾µÀ<¿í
´ôi@!Ӑ¸ŸnE?ú"âÀ*'?Á§¦b)ë·?¨¦ÜOKÃ?éÐ_Sw¡@à[\È
¿ë"m‹?ïýä1m`V?චpMoõ?£S=ÏÕ|¿èšˆҜ?·ÊùŸ$QAGNbllWN B0343.1+8247?ï×^(¬œ?qÇ5(?Qƒì¨?O÷…MŒ‹a?oßá×ÇYy?n7ƒ"bû?߿"?Œ÷"‰DÓ?NB,þ¼3?aêMpŸû?ˆy3íoóB?Šl¹eª¬?îí³ûòÍ?ª·S9e?{¨5""?u!£F®u?«L0@»?Ëî‡?îÏ/º½?Š©º]Š!:?zÚ·['?savˆ?ŸfGё…?ˆá k¹4FGL J0354.4+4643¿½ÄM¯úôÀ"¬ó±³À9,ó*.§³À;˜ìÿr;‡@@õÜ»'M@*º:#?¶` ¦Õ?¼ÃÎ!`£@§Å¬G@(BÒ¸t%?íQ5aáœh¿âY>?€Éi¿èw
bZé¿äœ¼cÈý4¿ê§l ½$c¿ðAGNbcu3FGL J0354.1+4643B3 0350+465?ï_¢'Ÿ}æ?ŽÐk‹Ã?\`ÁÇ­¨?WÍýØOG'?'E±/óÈ9?%Ò$¹Aí?ì(Ä̝0]?»þQï^'v?PwɃ
.?`,6"—?¾wúu
0å?»ç‡{‹z&?íÁVmoP–?—Žõ·Mÿ?"ôˆDhË?x:ïP—¿c?®­wãœ]?"Ÿü~îÝ.?î; ™V›?ˆÕ²Û±[?… Ô¶÷Eõ?l#Ä#š?¦ýÈجÄÛ?†Sôږ4FGL J0354.7-1617?áÅFsàUÀG)l?Ä;.À:û|üªàêÀ<€ž @I¥Î0O(@×N›n…ð?͆-—¡?³ÓÄ[d*?áº}ibD@"hMò&N?â"õbîâ¿áuҟʋ)¿åw©Ÿ¡—¿ç‡¶"v¿ïÿ•Âû?è½hvAGNfsrqPKS 0352-164?ïéUÃbG™?^÷‹‹?0¨‹fÐ)?'Sa¬¾?d•;ŒKŽ/?\ÇÝ>Ç?ï‹W?§5?ŠòÎT®Oß?B5…|ìg?Xöˆm"Ÿq?Œ×Äq:?‰d±C»Ïï?ïž8k?€:í¼–›?iÙoƒºB?ZBKÁ^~?›Ã^Nˆ{8?}(©1ÁA?ïÅmqPì?dô:.¸²"?7ø¿ÓÇ\D?+OX°Pƒ?{É»'‡?dvüç݇4FGL J0354.7+8009?ª'Öä3@4á?J˜«À:[í£)æÀ<–!à$˜f@vlÉ×Ïà@SR"Ã?ÀL"½ê[Ô?À¦ÿVýé?ûpû€>~Á@tP¬ñT?â­ž´5§?Öë©|Åñ¿ã"_½Õ¹¿åv·'"…¿ä»¢£-—¿ëKf/ßÁœAGNbll3FGL J0354.6+8011S5 0346+80?ì™*è'Ј?ÑSR	fX ?NÝÍS‡ó?UÔÊüÊs4?ºøí!BkÞ?ÑW7Ñ?ïÏ%s¼Ä?x¯ðì	³?6ê£ÈP?MÂ7LpvÓ?vþ›å'3?w3³ûÀ>˜?îæ4¡?ˆUüNmf?t¨ÝŠÿ^?gƒâV×d?ž3UÆ	ñ?†‡Ï?ïõ
X
ÅÞ?DÐA_"?(Í	6øæ?WzJšf?RѮÕAÞ?DX¼>R4FGL J0355.1-1841¿Ùß*¿¾"ÀGËs2'À;?¦½oÀ<ÇQâJãS@ Êæm²¶?ý6Ó¼)ç?Ñkúú݁P?À!hE
Ñ$?짧¯i?ü¨ÚiÃh¿í(¾ÐŠÇo¿ì	| ºu1¿ÃP"'5ú¹¿ÕEM\T>Ç¿ïхc¯˜?îÉ,«AGNbcuNVSS J035513-184309?ףּ¡Ï1^?wÖ]n?BÙ>€ŽT?Cªi47\?ƒqƒ¤*°?Їk9?îúù7Käá?™auAi?^ÛÞ÷Hî%?k@NDzc?ž³'Ôì?—:æ•r­?î@?yd•Ëí)?'øÍcE?z—¦§%^?«1‹Ó£=l?‹¶b¿Ásü?íæÉxY‰?—Ï%óTÕ?eK-ÏàLÄ?_Ø
»±²P?°%pE¾1Y?–™GKç·4FGL J0355.3+3909?좠-SíŠÀ&uš¶ÐÀ;gÐâÜÀ<w´ÃÁ‹P@"­e«£?ü¤
5ãè?ÐáÛý—E?¤l…~	?ÙuJÅK#??áÀÛ'£H¿ïêu¿Ÿ½ ?ïþÒn¥Ð¿ÐœEÛ×V¾¿çšãEµ¿½TfÈ{"¿àÑ(l0AGNbcuCRATES J035515+390907?î€ô‹ü×Ë?¬}Î^Š¡²?8ƒ©8Êr?=–%½,ʈ?§À 8àÇ?¬hœVã
x?ä‡ÄfD'Ú?Ҍr
Èt@?‹g‰»5L-?¢f9WÌ?Ö:å1ë?Òs´+ý+?ëÅ#É?¢w¨í?…³
oƒô"?xŸÕ?YuŸ?¿¥™O-?¡dN,ÊÄ?ܔl1÷?ºý¾&±E? º¶IM2?ž†QpP)Â?àªPåRžc?½B¸ø$©Z4FGL J0356.1-1329¿é`\'{hÀFq[ÕìÀ;,ÓD¶vÀ<µ}¼Ä@´HÔÛ.?ÿ<r\=îx?Ñi·¿Ža?¼nvÖ 2¥?ëw "~–@a[0RX=¿í€
Fªß<¿¶Ê=ü9÷È¿äüYòŠÌ¿×xXKo¿àKs2&Ä¿ïöÐâC6AGNbcuNVSS J035611-132908?ﯲ½å ?"ú#îŽïP?;ZXfã¿°?NÛ9G
Þ|?ƒ8¬MOyÝ?"›$n"3?ïc»7Y§?'W
{º]?>òšÅƒh?J69ŒS½?"%dΩµ3?ñ_)}?îgѨV+?ˆ¸èýÿ:?o@üGtª{?VeËQ¨É,?§ŽÕ¶&?‡"@!Òv?îø÷>ãe?÷4òa‡ë?P`®ÞÐÞ?Bhjo@?Ÿßr±†D?êÖW¯J—4FGL J0357.0-4955?Þ¢O‹ÑÀH	‹`ñ²_À:˜WšÀ<žßVø4@]ÁÒî@¯!Áçã?¶Ùã`·û¯?·!ÕgÐô¥?ÿ3;C£@^ÎTsö¿é‹fe¦Ò¿Ñy‰¤*¿âÄãß»¿ã™ã€îR¿âĀÍð¹¿êv›r·®AGNbll3FGL J0357.1-4957PKS 0355-500?ïNÞF6a?"úyæx!¸?ekŠ­2vE?`[äT'è?šè²á'å?'òë%ä^;?ïD;Ă? UxRDO?\mNGìL?l'ëÚ¦<²?›ÕB"ªà?Ÿû7D9"?í-ˆÐ$Öï?›&7Fד?Jz mMì?'P²¥¢ð?²ö½õ
?–þÍx"+?ï/ØI«ÈQ?€)~z¤_Ë?zÔ9
qnú?hg(8?"Oè‡*š?{ÚÑÀ4FGL J0357.2+2320?é`ûC
tVÀ6zÞÑ·À:ŒÄ¤	_$À<Legbå¨@ùþ«@ÿÉ^ƒC?Â8‰‰V*"?¨<S~"j?çسiy@ž'¯jfP?î0A`ó_ß¿ßztÛt/}¿éƒ1èEÏ¿ØӦύ¿ä¸é@ ¦¿ëL°/bAGNbcu3FGL J0357.1+2325MG3 J035721+2319?î}"S͚?èMì+p?tŠñÐ헏?n¹ÿ«;"?¥–\‰¤?›È'0¬P?ï{W$©Ç?–=—Ftì?Z!±À1?b´¹'x1¢?šðsZ‹N?•\Dþ\¦?ínºù8Ç?–è$ö‡ê?÷Ó¿Û9?mZY³bj?²K4þ>]?•É"ä°?íH'—éÖ?'~#~hUõ?Ž·Â)ñ¤?v{ÚQ«¦?³žÙrûs?yʉ?Œ4FGL J0357.2-0319¿Æ^iž:y_ÀCÖb^™éKÀ:È5A*l»À<]IfË@!›ÖY¾bQ?ú³Qf$!G?Ç×&—ïJ{?Ã
pÖ×½—?ýÅÆHNMk@†¼
Ý©"¿ïÿ^Ê¾¿ïƒƒwï$æ?ïÿ‹Á>Ï¿á§Áåèý…¿Ó¦¶ão+¿Õ,0àr›ÿAGNbcu2MASS J03572609-0317596?îû_Îgœ?—Kû™A¤O?I©±"\o?Gþg\À»-?ŸÆҐ)?–ï¼……V?îýyĆ3Ñ?›¢iA/Þ?SŽÞΗ?a GsWª?Ÿ®XÉ
?š.æ"òÍ
?ísÅéH?œ¯{Hg?rLG`ðø?agÅòZP?¶—Z¦²n?›ÜlŽ"¤a?ë†àuì€?¦Ï…‹ZÌ?[w²|¸ ñ?Zkž.à‰Ó?Á°Ý.ܾ?¦Ââ )…×4FGL J0357.6-4625¿âT¯¸GÀHd\6fÀ:äÜüŸÜÀ<Ò´%t@ô¦›µ¨™@³'[·¶»?"xŠ«?3?®ªc°y?ëGæ^d%@#®ýY¬?ïíZPü¿ÙúsCn"³¿ä³R"ÿÝ~¼¨š¿é"a å¿ïÝDuAGNbcuPKS 0355-465?ï-r&Ë??•_È7¯åý?desØÝ\}?\Pû× D?™Í£@
ì¥?"q±q«ïØ?ï@7ºI0*?"®:ëÅa?LÒL4ÑÃì?ZÚiÓNôê?—vU3lÄ?'õ¢bcè?îŽAˆi?'(OÛù¶Z?]hg–ª?rĪ4k?«£•Í"ß?×K%A³?ï!;ÝJQ?|iÛ@Î,?xgµ¦œU?a²ºQêí?•Â˯¯Ä?y«Á‡×"Ç4FGL J0358.0-6946?ÜÈêŒr·ÀCÛá2µ^òÀ<'³1fªÀ=Šlê&3@˜<%u/'@|x £?Ý}Œó˜ép?ï>ž¦Ÿ@ÍýAÞÌ@…*ÁõƒO¿êÝSb}£š¿Ûí¼[t'?–"MWÕ1©¿ã³_¿-R¿ïüz¿ï—7z>ŠAGNbcu3FGL J0356.3-6948PMN J0357-6948?ë™2^´ï?º÷	9?¯'¾\—B??°ïŠ»uì›?³¢á.·s?°#¾ò/³?ä?ò\|¦?̶ÏâU¦?ǨÙ8ùžë?ÇÁçdÇ#§?ÇW]Uæ?»pcš«šÞ?ædz¸Ÿp"?¯#ºzôa?Áuˆ+Áô!?¤»ƒ3:'¼?ÄøŒñÀI"?¤!r̾£G?ä!@Ed?¼9'xv"§?Лþ{êð?¹?kã<µ?¼žÿh) ?³tpSO¹Â4FGL J0358.1-5954¿Û	U`§ÀF=žbV6mÀ:ëIBi1À<Ïs]Å­õ@oéò¢t@¿Š:›?Éç<t$•?ÁŒwG4G?ñíÏ`ûÃZ@oûe'?ïýfȋõl¿åÍEbàŸè¿â˓¿å­÷¯î¿ëÒEb	àT¿ïÿôw5ÁƒAGNbllAT20G J035814-595233?ï 4»@?Ž\C°Q—€?owCt.D¨?dÁÒ_5x?˜
±BÏy?ŒL
^w)?î©nÁ¡HØ?œÙ"NÆ?eh[Á¥(‡?n}Ø@gs?¤Ž)Ñö?›Ä/ó‡R?í¦rô†öÒ?"E\ãÐ4?Œ":†Ã¹+?€Ûžv3'S?®wÂߤº?~BV–¸w?îP¸7R¸?‰W³±=vw?‡83Ö`ðè?p‰NΌ†á?¥&o•G¸V?ˆ^ÿE¦Ê4FGL J0358.6+0634?ÝÆ]'+À@Èك"t—À:6
fðÏáÀ<
$ÜX[@ê+‹p@¨÷ÛnP?Ç.ìË?É1‹þ¦c¬@¯/:€.@‰!.-?åkì O+¿Ó9€TN6¿é°"òsP¿âü^pпïÿþˆ0»Š?ïòF~"…‰AGNbcu3FGL J0358.7+0633PMN J0358+0629?ï£þL¨vØ?¬é"½ ®?eaš=ܜ?d/:ÇRã?¨%¯RÒî?¬ñÊéz?ïWói?–Iƒãz)?S숆Ù?kÃú'žü?"ÏÓD e+?"ÓÏV?í•*ð¯Ao?—þùuµ.ù?jKP/
 ?ÌÙf13?®x+Lôd?"‰UáUð?ïmŸÄ_"Ó?ztP.½?\ãê拐?Ljm'@?}ÈÅ®|Õ?xù­M´èØ4FGL J0358.7+7649?àuxþwu@1Å÷@=ݱÀ:ɬQ,B~À<¡ ÔƖ@c/p0?ýÑÍ¢µ¢?Êm®Ú˜A?Òc¢ýe?þÆIàô¡þ?ïv%5;¦¿éÔMdº¿â£˜@S,M¿Í5AU_ØÙ¿â-sk1§B¿ê:êýdo@¿á—}à€ˆÑAGNbcu3FGL J0359.7+7649WN B0351.8+7640?íc¾09J?©×°'ª?Pl¶?‡"Z™úâ?°ï߄p²Í?§GŠá'Ø?ç=¶>Ùæ?ÅÝéŒýÃ?½
?ý-?½=¶UB|?Ĉ e…Õ?¼¯¥µÚŽ?êFã¸}ò~?£š·:Ƶ?®GÔ\WrI?––êq‹~?¾¤ø
ä²ë?¶Ÿ{ø«ë?å˜âmÔ?­.Øpä?¹7¨#'?¢²š£˜™?Ídêæ6î?¦IDZu®!4FGL J0358.9+6004?ﴅt.â'@°ºë#À9§)£gxµÀ;®êÏS)@X¥¨¼@}ïAkÛ?ÀG3å?ÄÒU7iù™@(
%ïû@Êú~5åë?ïõâlvK¿Ýˬ&w
¿êãÁ¦(U¿à‡‡émíC¿ïòÄBº³?îI"~Q¿AGNfsrq3FGL J0358.8+6002TXS 0354+599?ïéxÛ©~2?bWûàWÿÑ?Ožµ'Pº?S1M· ?]?ÒBuÓ?YœïŒ9?îAÁ2Qa¢?±ÂÎÂÛ"¹?YQ¸7ۖ?sY 'Ñá?«cå(&ù?±Mñ"̔?ì|øå)´Ï?Ÿ$‡Gu?"r²½â{X?"™q,þÍ?·;Œ'9º·?›MƆãür?ïo?;א?|yŒ_+Àª?cٝ9tÆ?X‹š÷åR?9É»á*S?y©!Ÿch¿4FGL J0359.0-3053¿í;`æÜÀHŒ¦ YŸÀ:ÖêedçÀ<«nñOc@ GʏÜ?ý¶¡è´?Ã,hÿ?³	ÊÀ>Z??ñ…Žd²1@@ó|ç‡8C¿ïþyzϪ?ïöþ~ö€$¿æ";ßT8ç¿Ó0êÄ.™¿á7u‰Ââ¿ØKéBNY)AGNbllNVSS J035856-305446?ïîi°{?X|7Ó¥­?$¥G{ˍ}?b)û·	?`L–Ø#ËÅ?Wź;$Är?ï³ãTF?†e\Wáxµ?1<Á|s?N#‰'6uW?'}FptX?…˜
žúà?îÙ©îM\?" óžl¼?f¡éû:È?S)À¥(Æ? ûBƒ
ƒt?ƒ€t
šB˜?ï{¬ûËû´?r…«Š<³8?SeÞj™þ®?CKP\r×Ý?Ž¨?­ÒÃ?rî©Å4FGL J0359.4-0236¿á·>"ØüÀCk=ÀTïFÀ;	3Ê1çÚÀ<gjÜì¬@!z²Us¥?úûÏÔ¿	–?Ñb{ö£ð?Éë~:R?üf\Ukl`@¡:ãUÐ?ïvé¡éÜ¿ïÿYM»?ïÿ¦=ìʙ¿ä|{±QFD¿Ãt0é×ʂ¿èèß½jY:AGNbcuNVSS J035923-023501?ì¸$'ºš>?²\?	W£?f°"^¬ã'?\°]¾tj?¹‰VÏ5Æý?²:M‰ývW?î‡eâëõ?¤¿ìðþð?h"x<?w[ÁZˆú?¦	i‰¿›¶?¢'íTæ?ìN®¬.÷¾?Ÿ¸¨{vŸc?'ÌrÜå:)?t*Öfž?»0üBëšÉ?ž- ¼â\?è`ôXò	N?²ú&¾»w?c¢n×
>è?c´ØÑbU?Î-¤àÛ±Ç?²ÿkÐ
ù;4FGL J0359.4-2616¿ï"«.*ÆÀH>›A:À:¯8lÄNÀ<k5îÏV@"÷Ô7z@@J@Ejm\?ńüéõýs?¡ˆ6ð¬ûÌ?Ù¦:ý,)@++àÖð?ë:kkˆå¿ãó$Oj¡_¿å··6¿àŽ4á‰t¿Üõ¡'FA¿ïïуjƒAGNbll3FGL J0359.3-2612PKS 0357-264?î¨~"Eš?™†"~­(ù?e:å´YÊ?Yë±¹??¤,Ôhp`Ê?˜ÍGLü–?ï
·WÙ*?–?Õº¦b?Yô'•îÔC?h˜#Pâ~? Ÿû¥íd?"Æ0u†	n?í´G"­M?">{·±?~‰p¼LŽ?hþÙ¬jˆ?°u,ÓõÌ®?'Ô&´3—Ú?í°­mUr?¾þÖí§?sž][WX?aX™1ha*?±EàÞ¿Ÿ?KøªÜ4FGL J0359.6+5057?í†2±O.¿ùqé¼ÇœÀ8$
!¼À;.•>Á@hDn
B@ÊâçÁE?§Hÿh^?¿×­?W@E™›@"Ÿe‹u¿Û­øᨦþ¿ãwµxó0å¿çlÜ×ÜËH¿éw>û¾R¿ìƓͧ¾¿ïÿ¸SåZAGNfsrqNRAO 150?]ËI?…ýò±+½K?dý¹iç?fø°)Þ¨?‡W·¡žÓ&?ƒÑïM'Þ+?í}éÛß?Âxó¤?H
—Ï¥Rµ?dîÝNa(?·sõˆ®m?ÁþÎg€ºÞ?ëðDÄø'?¦\¶]?¡•)eé?"§wru·?·ñÛÿCˆx?¢•ùWñÀ ?ç2Og?v†~¸w(Â?Qüà'yÕ?Em›Z 2?‡šª.ˆ·V?u¾ÜE¹3Ë4FGL J0400.7+3920?ڗ̌­o\À$o"5ÒIäÀ:-idÒÀ;£J@·?ñ\¤@н¨"?ÉӎG€ó?ÓãùŒ|{?öWþ>^à`@&èãÙ®³?]ʶr¿Ó;Z^›@ä¿Õ9ÐfqN¿æ`MÈá¿êÔ­kÞul¿æ¹£Ÿ×Ì/AGNbcuGB6 J0400+3921?³µ'·<EÎ?­¿_÷ß²·?²ðòº··?«@·KäW?ë+<±Á"Î?¶bÇ O?Úp'Xì&…?Êßøoù†?¬¯Uq6ó?®Ž;I÷%ý?àüÉ|x9N?ÊfìÁÈ'ä?Ù΋:QG?¯%Èí?ÆLÞ.aª?£ÁÇd½7?Ûr]"Ù¹?«á€Ž9…&?Ûèw'.Øë?ª©Yÿƒ—µ?ü¶,YÏÊ?¦PaRÐÑj?Ú9-g¤?0?°ƒ]kYì4FGL J0401.0-5353?ïÂdÊÁÀG*UC(s½À;NXø¿™ÞÀ<Ïq¾‰=@!í\MÞ°$?ùr_µj?ʏ˥†Í?°Io	Î
?晐?'Þ@ƒtük¡?ï×£ -²k¿äRW…øÒå¿âW˜" ;_¿ÖÐ5'BåÙ¿»F@V1dý¿Ó5½|!åAGNbcu3FGL J0401.0-53591RXS J040111.9-535456?ï®î ,†?}XC=%/?4	‡ÉÖª?-1µ›6Ú?ƒŸo°ö?|þ†Ÿ´X+?ï_q€g '?"Ü4›ãW?FŸWly?XhNf?"`êúq?¶?'B ‡`1‡?íËÆýâj?– ˆXè'?h͌,`Ô&?U¨'Ù»?°àíf­æ?–?éí\´ë?î	Ük´®h?–—ž™ #?T"¥NÖ¤i?Owt7ø	?®½œ>dK?–)ëYîÉ4FGL J0401.3+0412¿è­'¥¸XÀA?Ú@RÖgÀ:>¥¸‹Í(À<
ïGK@7A"@±¤RZ@?Ãq·<íœ%?§cm1µQ?åujæ'è@y&
«ª"?ïÿµÂÅ¿éæ)«0ñ¿æq´]j>b¿àïÔ;V¿è°a&‹…¿ï÷¡Œ­"
AGNbcuMG1 J040119+0412?î]€ú|FÞ?¨`ÿ²l8I?r77¨gm)?lˆÎsjée?§á	c.¤?§=mféYN?à"­o?£A,ä
?aäÅh\u?pD1Ÿ¦/?¥÷õ¦®£L?¢tåɨg‰?êÚóŸ"Ý?§!qV·`§?—Ââoõ?…94ÞBÉ?Á›ÕB†Œö?¤›+PVR?íÓŠ?•'!s©]?'Ke­% ?iüi{fyD?µú±—_
?"Èû£÷4FGL J0401.7+2112¿Íñ-ÙpãÝÀ7?uÙ ð¦À9"a#0†±À<ä)à¤@ŽzÒ.5@G6¥®zÒ?±a¹ƒnßÝ?™";$³Ž?äêׯ~Þ,@9¤=Œ}|?¢0ž@¥ë¿ås´È¿çb P‡Ø¿ä¥U~Ž¿å°ÉaÕ¿á=u¬T‡AAGNfsrq3FGL J0401.4+2109TXS 0358+210?ï×tYÞDí?tZ͛kV?8™‡¸˜ä?4"¤' øÀ?r¼:•T	?sa­ÇѳÒ?ïÝ9Vµ·¶?vgóSƒO¡?!?¦8‡xm?BÀÈk?pÙWs_éf?u1,œvß@?ï¤!6	?'ÄQR§E?jïX¦Uÿ‡?Xõn‡¹Å?š!Àg~ã?B7l\©?ïå®`uW?Sl6[Qx?*_G͂*g?Œ-õ?h««
ÐÜ9?RotÍqÑ4FGL J0401.9-2034?Ç{Yι+ÀG3'äKoÀ9Žn™:Ï	À<]ʹÍÈ@UBø";@'<O;§v?¯Ïbpãm?¬© Øà?úð¥)œ±@1ûЛc?ïîíôdÁK¿â*^x[[¿ãµo¸õs¿ãa.A?e¿ê\w?&±p¿æ=¨6ëN˜AGNbcuPMN J0401-2034?ïµýÐGîT?‰6Ÿ«t4?CÞ^1ªsi?G;éNÜá?B¦
éÄ!?ˆxòð,§Õ?ïÌôGe¹Ø?PEqí¿6?*´§±eÜ?B…'¬•"?x°;—å‰?~­ó»šê?ï&ó¬Tm?€êÌ?pž[î2þz?iAá¤O››?–ù󃲮?~]¾€.`ž?ïð֜1'M?JÉ}¹ro´?5ç~ãd;?*ÖdEÏ
(?XØ踍Ô?G•Sפ^4FGL J0402.0-2616¿ïþ¯9'Ç_ÀG׍÷¤ç«À:'C‹p+À<4–åŠ2ô@•§vQ?ÿëî€{»b?»§•/Ҁ–?ÅÒ.
ªRú@
«Ý3L]§@†Êk°??âk6¯Æ,?'‰ÇПÑR¿ßˋ¤cw¿á‡Öޞ†h¿ãxUFƒr¿ïûþ~ÀAGNbll3FGL J0402.1-2618PKS 0359-264?ïÄ¥Ò*'9?.Ên'Ñç?liÉ5 øÅ?x`xÕ?nðd MϾ?fµŽú]ª?ï$ËQ¤À?—ÿ-:(›m?S˜Åó‹H1?Zº>îë"?š-	nÒ³b?—ClV}Ã-?Xú€?ÿZ€¥Ý?£WÀø¨?~#‰n"è? Fáª2S[?†VáD—]?ힵhÏê	?{ƒþ!K³?zg¦ÏÊÅð?h@i‰U?±cÚL"X?ŽìÄÚÚ4FGL J0402.0+2737¿ï¦nýlZzÀ2¦•BCÀ;yD|	À<[Òç™í@¶†ƒ<`@`Ù¼ŸX?Ê(y›ÍP€?¡Ìud8#?ÚÛÏÊ@ÃŒÜÇÂ?îÏËOKE¿äùˆaãÊÀ¿é.f f¿å+§'i?‰ÄÔcw§4¿è…#ÀÏhˆAGNbcu87GB 035856.9+272842?îŒPiŸ?¦d&, ?mä4^0¾?——j÷•×?­ø÷¸J?¢Uäö-I?îý–—G—5?¤!f¬Oê?`o»¢??wɑ…{ƒ/?ž?5¢Êq—?£+‡7ÿ?ì÷Ÿf÷¬¿?™µ<I¦aV?}þ1øžŠ?mçP¬L`c?¶qÄå#?˜½úÏHyê?íÏÙÔl3?•&ã]yr?Q£È&ëäH?N Jpµh+?±:¢<·'?•" |†4FGL J0402.1-3147?Õ&4¥ÀHEmã2iàÀ:OŠÞó­À<œ£Žåáq@nf½¤:Ý@D–eÖô?¸q¢"¤¿è¿‹è	û<²õ?Òm˜ŸH°@úþ½_Çf¿Êop»©äÀ¿åƒd£î‡¿æ=E¥ü~k¿àŽ1@¿¸½¿æä"pB]¿ïÿÿ" 5•AGNfsrq3FGL J0401.8-3144PKS 0400-319?ïÂj¤TÀ?|¼-~µ?LûHêºAw?@ˆA"8?{+D¸Ho?{¤ÖM':X?ï²m´c?‡
º
*g?3@`dkTL?J³Ã‰þO?'ʏä
?†)	Û7*?îÍ÷ðByM?Œ¬DHùðg?q
¼-&•Z?b§Ì—eŸý? þÉv3˜k?‰ða2«íH?ïÈËCzq?al7Ex2Í?WðÇQ]?DÞ^2òüÂ?u÷lnp›?^5µW°ã4FGL J0402.9+6433¿í±¦k$^@!Ü¢˜E܃À;0uєÀ<Md;é»@!ë×ðÂJh?þZj)i…Ö?ݍ}K…:?¬1ž!'u?¯7Ö°ü6È@œ^;Ÿ"Y?ïûŽ¶çˆ:¿än­Aí
Z¿í~³íQ¿°@ô'âÁ¿Ï^z·¬)¿à¼-BXj$AGNbcuNVSS J040254+643509?à›+"Sãs?ʄ#ñlà?a‰KÌe?m¸w"û¹ù?Þ§kÄÀ Q?Êw":YHŽ?Ù "']?Ê4›gþ>B?'žf§[Ž?"$F?	ò?ã*öV²Nä?Éãø'Û"¥?çbCñé)?§lyí¨‰A?‡ñ-ÑÕ¢?sx,JIJ?Ð|lö­žÿ?¦j…ìBâ?êYÜÃá"?®'qÍëó?``j2?`Ý°"×Ùx?ǒhˆ¶ø?®Æ¸9¥Û4FGL J0403.3+2601¿"¨^ýœÀ3—®FÏÈ*À:uêe:íÀ<"Š•Ø@—ÿ-ól@D@¡±?Éò–J"³ƒ?ÑÕÍ\>Å8@ÐP_"äN@½¤ܘG?ïþÙY£	…¿ç®yZ^ñ'¿èǰބ°(¿äßS¢"j¿ïÿ÷!	:?áê8ÅCAGNfsrqOF 200?î6"E9Ð?£'ñýûâ?"ZFh飛?–Dqé?¢òº§7'J?›µŠüBÞ5?ìË÷Å´§ñ?µš>ŒAþ-?œzðK…š£?©ðËF}mÉ?²…¿yYÒ?¬ëŒ8¦z?èÌ à)½d?©{Úà‡àQ?±‹¯4 ?—²œ±9¤î?Äñ§¾ºb?¢±emáð?éÚ¤Žõð2?£";ùÁ?¥%°_+–÷?‹ÆþQ—?ÃL¬]Yx? ù̔L¶04FGL J0403.5-2437?ãè ÍëZ×ÀG{SÞ¤e¥À:|%«‹3¥À<†:8
3@Fëˆúÿ@^®&˜}?¾x2–«'¶?"Úâ»x3?Ò)["æ^ï@

åÓYü¿ÛÖPē˜N¿ãòT{'W^¿ãn=Mh¿ét÷Ãñ[ø¿ï¼jÿR[?îÔ1°|4.AGNbll3FGL J0403.7-2442TXS 0401-248?ïÎÒq?rÓ?x8¹Ê©?DÔÊ[±f?CbAV
ñ?uü.ã@;?w\Hgvÿi?)U}?ˆÕ'g( j?=Ӂ‰?O¬ør¿œ€?ˆ-"Ø+?‡­šGŠš?ï'}<ä\?‡s
¬Bç€?zûâ ©X?|L°â›PW?—N·°93?wàµÃÞW?ïÒL·Ê1J?dnQ¼múl?CÖvÞú9?8•j³ìp?tw©L{=?cP_æû‰4FGL J0403.9-3605?àí¨_/:€ÀH=ÄڐïÀ7R}hájêÀ;¤eƒèWm@j/™@%Ø{V¸?'»˜¼'…?Áœa_–h@*9AÈ!la@!lð—'=2¿Í`ž—i¿âäZB@Â=¿èt¤Ò²À¿éj šª:Ò¿í@j‰
Ö¿èãD]}¿AGNFSRQ3FGL J0403.9-3604PKS 0402-362?ïY1"?«
¹ç?|ó÷jIÅ?'žó"Z"?‹˜D¸;?§Åâk4£?îå®–p•?ªóÛ6®—'?o¤±E aÍ?‡•_ˆi¢?ŸU§"}á?©<^'J1ø?쒰ó?§7`>š¬?°Ï *Ï%¤?¢ÛcóÆl?¥6¶›0#"?™>0N¯ž‹?ïçó;dG?c*¦®áU?QÒîõ"L?QxL4‰Ì?`•IÚîÀ?[sè(ø4FGL J0404.1-1715¿î@¶²ÚÀFJ5çB™ÙÀ;CTxþŸÀ<Ì۔ìÝ@ )–ˈÿî?þïÙ\'HC?ËÅPV¯$?«—á€"‡?âTŸ^Õxm?ýQµ§—38?ïË$V ž¿ê‰G;þ³Ð¿Ï¨£¸+€¿áãÚÀ€c=¿ØÄúptb¿ä_@zAGNbcuPMN J0404-1718?ï(õ.È}á?'ˆ®^D?FÃèŒFÐå?;ŠûÑeK?š+:âŽ
ƒ?'UR@—ö?îîÏßbñ*?šò×Ü1¯L?Z'sƒyŽý?kÕXÞO26? >vmµ ì?™ù܁Ì?íØk%;?'àC«ñ¶p?r´(d€¤?a•ï+…	?°º!¦Í!?'G§§Åu?ìðJ\‡}?—,Ø$
AÜ?n•o¥âê?b
hù˜?·ŒÈpIõ	?—ªº9Jô4FGL J0404.3-1559¿Ñÿ·ð
®IÀF
–_RuïÀ;O²——aÀ<ÁR¡ƒâ@Žèc¬!Ü@qL"îA'?Ô{Á!Gù>?Ó,Kb~û3?üBkK @$ñ[Í[=?ïëÁ¹É:?Ù-«ŸU›=¿åSç]DZZ¿×õ¡Ø,|¿ïÿúŒ—Ó¿è—Ý÷vÅAGNbcuPMN J0404-1559?ï´ßØÕ®?vÞNͲQ?_…ÒgêT…?W±·æu§?}¯ùš"5?t—!]¥!!?îñªêTˆr?™EªÍØ)?c:ä>—cË?qû¸®ò«?ŸcF-œN?–ãå'Æ/?íSÓ'CP?"¡½)Äü–?˜.x–ì¶^?ˆ8Ú3_…?®«'@T¤w?Ž¾û}]Œ?îpíÍ^7?ŠÖܗ–±p?ƒ9qu%ü"?vìõ]sÚø?¤"ÆÌÓÜ?‡Ðþ@¿˜4FGL J0405.6-1308?ŠšîÆÀEPíÍ9ÚÀ9wdå\æ‹À<KãýjúJ@oâ˜»ù@sÞÚŠ¬?ª»=RÏ¿ŠYE¢Ë?ÛÌӂÉs|@ƒæ2(œ¿Ùʦ¢¿¿äœ´&†'¿éz¡†Íå¿ä9Qàd)¿ïü'¶vI2?ï×i©âAGNfsrq3FGL J0405.5-1307PKS 0403-13?ï÷$Ûl48?Zïo' å?+Äêó4Ä?;a€rÐí?L{WÇòQY?U¬/_Åê?ïÄÙµâÊÐ?‰•ÛÂQé0?.Å&œ8?GºÝ°ßA?|œûÞz"×?ˆËœ! `Ö?ï@ñGÃtO?€)­¦ï%?l;ˆÝP?eUys{(?"_ϖZ¦?|…aÎ9é?ïö¤VFó®?C†xÈ1?,ÓÔ©I}5?#®JºI¡?N9±¹Þä"?@ÿduæ¼Ù4FGL J0406.0-5407?ïÒÞO3ÍkÀFȒ£"¯À:àŸd´µÀ<±2«M÷@«ó[VèÅ@¯àè@?Å
ÈÂ|?¤Õq¶ü€ï?à_o1CD@?ûH
ZÍ?ïæW¸M¹Ç¿êË
å›Ð«¿ÚƒÊE‰ø¿ãð'~Êá:¿éž%"ôÆç¿ïÿý±q&´AGNbcuSUMSS J040608-540445?ïÇn¸¾X?q©ÅúH
?Pm·‹ß¸(?FàÖ\þ¡]?x-6
¨æ?p^çîÿë?ïVtTJ~?öâ	@_?JÍÒk}²Ã?XýmãÞ*œ?"[ãTO4?ŽyïµÝZ?íçÿ¹Ó,p?Ã¿›'?†ð1)?~‡Kùpã?«ßˆCñû?‹ҙL«E?ïBÒÔ7ö?zY½»~?pr#×#OQ?\JŸÂhÍÑ?"‰ˆP-u?xDž˜4ÜÌ4FGL J0407.0-3826¿êáÖî(ÀGð:}ªOÊÀ8'pûëžIÀ;ÌÊ÷à@ÊÊÁ¯¸?@øfC*÷û?£w£%o·?¼¨ËæÙD@ÿE™›@Y؍Ë/>?èP«Hî†[¿ÝJŒL˜_¿åÏÞú÷­¿æ^ä&…¥Ç¿é!(n´¿ïþ'jöîßAGNfsrq3FGL J0407.1-3825PKS 0405-385?ï '˜_Ž™?{ä0£(ƒ?`Økê28?UžñrL?ƒ¿þíÔë?y‹ÉdÁ†?ïO]ÛÍÚ?Š^€ËMŒq?Ka˜" ?o,µP`ý?Š:Âo‹a‰?ˆ'f{Ï?ï
Ýݜ²?‹ñ¨g*?~¼ºz@©I?|û"ó'ó`?–õ0¥¼?–?†CPc¢8p?ï·v8B?ku#º°?XLÐxªî?Nҋš¤ké?~1ÃÅÆ#g?gß+nR~4FGL J0407.5+0741¿»÷¥œòÀ?$GäÀ9U¸éÀùZÀ;ëŽÑ¿zÕ@Ç=ûc84@Wn{ޝ°?°Øú''–ñ?£(:[ÆzM?òqV8ú@½Œqg÷5?î 'ódK¿Òý¼-î%¿æºUÑ쓿ä5ëß·‹¿âû"ÀĀο倴%6nAGNbll3FGL J0407.5+0740TXS 0404+075?ïkP"víw?­RšXHÂ?Mñƒæ²?D0ðxiÕQ?'¦o'ñÓ¦?wjˆÚ5?{
E?‰‡·b2¢‹?@)F'K˜µ?S'í>ŒQ?ˆÜçùõ?ˆ9DÙ1é?¶ÆÚ?b!l¢_m?xa@\v˜?oH Å?¢˜¢–8?Œ¾|zïTc?îûØ­ÜN¤?~D/Þ`Ï?uúÚwò1?a—8"†Û?›3¦±®Ý?z˜æ7}4FGL J0409.4+3201?Ñ­¬¥SÐÑÀ,»"F™A…À:j«¾_KÀÀ<L)'ÉÁ€@ aùkç.Î@XKä ÷?»`¥_?¬¿n!¤H&é?Ö`½Z?ôÁ­]è?ìw~¼ž¿ééKRä©b¿àA|lb(ê¿Ó†_!£"¿à`¯"#¿æ'z-ǪAGNbcu3FGL J0409.4+3158NVSS J040928+320245?îó¬&k?"LY7?€Ï?eàï)8?_^AAõ½.?žç‹1Ô·Ð?'iánmß?î?šQU?«›ñJ Ø?s+‡ùÿš?€Äçñ7d´?© î‹	à?ªGA¢òÕr?íW³óXŠ?–-êÚ])*?9ZØyÂ?ošã9®9õ?³NՂ·´?"ãåZŽ<*?çŸcYæÓL?¤W]J͓?£®Ÿd=w›?‹¶Šö"ð?̖ʿUTé?¤f¬"Ï4FGL J0409.8-0359?܌"Ž'ÞÀB°€Ç:¼"À:0î'hÀ<K.cÀ™¹@¯'aÁæë?úօ˜ZÕ9?ºê!Fv²?ÓÛgšC
@ý+¿¡k@ö0툯?ï—ÆZÂÄ5¿Öµžþ'U¿Ë"Îš¿ßW
:M"¿ç6Ë£×àý¿ì+½óëõ‡AGNbll3FGL J0409.8-0358NVSS J040946-040003?îæ
·£#ä?—À
íØ6?‰ñKÇßý?†z߉Æ<?–E£("l?PS…ç?ï22_)¶?–}r g·?Z]BW¶»‡?i¾¢[~:?˜ßø¿]|?•|ñë]?胭h?ž?¯ô̞,¶º?¾c)€–Úš?§'ìGg?½k=l4q?¡žS$wc?î[T¤úÉÝ?Šµ™êë?r^7À5¸?_›­é¢Ô?§þî¸A{€?ŠŽ©e'š4FGL J0410.9+4216?ê·f»ÎÀ&Üã›EÀ9t»=¤¦À;é?l&š@vI±ú¹o@ËN˜‡œ?¶®#ÿ¹‰#?½ÞúaZë@î"þ"?@X1` (Õ?ïµK;gµ¿Ÿ¤,€Í¬¿â<à<Z¿âÊ|ûÔ!U¿â¥É㽿맾ŠßÂAGNbcuB3 0407+421?ï>\µà?•)P~'nç?Y} —%öÆ?Yþ¢P"î?–œ«Ñ l?"ž0°™?ìô{üuÑ?¸Qö&[Ú©?P#£û.‡…?h5΋V‡?¸™8/—Q?¸/íŽGÖ?í›äo8+?"Þ"}¨1?Š¯("Þ"?q
öA2ò3?°õ²÷sÂÔ?'G¥s§Ë?îyMÈmˆ?†xBí¥là?Ôº¬^Se?kÇÓ
?£õôԁ'²?"gb·Óy4FGL J0411.7+3041¿ëöÇ{Ã߂À-ó—»s5À:ÃÑðøüÀ<#AՍe¯@mqÕ‹@pÈ¥ߙ?օÞzt:?慍Þzt@oçáüú?þä#›e¡š?ïäÊ"%¼?´'ÿ¡‹U‰¿áˆÞ@<±¿éÆh¸P>¿ïÿ}#AM¨?ïû?!ÎAGNbcuGB6 J0411+3040?ìF(
±¥?´@Žâ_5P?² ~!ҝ?°ÑmŠ4•?¦\'ä@Âu?£LD^çt?ã£Àª»Z?ÑïB&N"?Ï-¢s<©N?ÏÃA>e?ÂCZähiJ?Àýû:A·×?äQŠÄpJd?¯%–ÔÐ?Â.[È"Ï!?¢Zj³Æ?̋y&P?©›³áÚY–?ÄÙ¹ñè¬?§…¨µ?Úú
ÝE<ö?¾ðÖñQ} ?ڙ)Æm?¾VP… 4FGL J0412.3+0239?àŸv…mg·À@™3]$žEÀ:4±‰zg¥À<³˜H`Â@r_˜ìË@b%#¥÷v?ÁZÌ)cь?®@Ÿb4?î"ЧLàƒ@3U#‡¿ã¿9+
Ë?Òµ)­xs¯¿äâ~—_®¿ã Þ҈Îp¿êŠDý`¿Þy–ÄÓHAGNbcuPKS 0409+025?íMtWÑ¿?©yK9óD?" ñ0ÂÙ?4û}Ìp
?±v7)1Ç?§^鵛*ú?ïsm%èâ?‹µQ ²è?B欀£n|?Oà€(öéÙ?û%úýÈ?Šø1Å+«?í6ðgË 1?žôíNl›?8ü	>Ö?''²°&?²a]>…Ö—?™˜ÍpÌuJ?î»Xpñ:|?~eSÊ;á?v'‰~ã%?`ý_Ïú—@?¡xGÁöu?|=Nm@¨x4FGL J0413.1-5332?ݔЃÝçõÀF\Ïkã}éÀ:‹…ÛÀ<QäJ—ÓÇ@±Šû"@/«SÖ@ê?µ¨Á?O÷?—°þ‡|X
?á`fQÒ@Ußêáµ½?ïÒéçÆ²¿âIfÿQ"¿çVSÉ«°¿åH¦4¿è|z¤áÌ¿Ý·Oµò–AGNfsrq3FGL J0413.6-5334PMN J0413-5332?ïØËNú$q?i)‹Zo?1fÏ%$
?!)YÎÅ"O?rˆ¢ûu?h¿ÿªfA_?ïØtd©÷B?y©5'‰%£?R~ŠÀŽy??š÷þrÊ?sHƒ°Ù\¦?xæ
U÷+?ï07F!?}¯vBÙÓÃ?g->«h;õ?TA…]Ğv?—hIÊ4<?zòr5°YÓ?ïôMÇ¿ˆ?Dg$7Ž?]«"ŽË¡?
!°a?V1‰¸8Y?CÚåòâ­ 4FGL J0414.6-0842?æς^¿~ÀCW¼]éÀ#À;W‹àsr¾À<§ü­e(y@àoW%Ö©@æ—b%?Ç鮄ã)0¿…/n=Üj¶?¿a@Œ¸	Ç@›2֖û?î©z¸-˜¿í;ž§"?'n6'ž¿æ¼ˆabñg¿âÙA…Þ¿ÔíUBý€ŸAGNbcu3FGL J0414.9-0840NVSS J041433-084206?ïZ'X?•ü‡€›·Ã?I°^}k?B_$rƒÕò?žQ'Íéš?•­TúS²þ?ï^À;²öy?'&Ûn
m?CP"u¨C?VÀsC?b?"‹Žƒ§?s˜ž´†?í¡¦™Z?•rŒ±½Ô²?t.pº¿y?i÷Å-?±¯è/‹Ëe?"kéá*:?ï,GÚ{Û?ƒ0ØÛå(?NSØVéÑ?D×(î¯yB?ž‡ÞýíÍb?ƒHÀp	Ã4FGL J0414.8-5338?ßñ»"o/}ÀF9Ç͉‹/À:ß´tç2ªÀ<ŒZ{v™@!Æ.Ü"?ú¿$º|?Él;½pc?Âu	ÂK"~?÷Dî|Iýz@¾ØR'ó2?îQí}ÇV?×/!°ÿ½¿ÃW—ULj¿Õ]ä·¥¿Â®9#b/Ë¿èg²GcAGNbcuRBS 0526?íÜÁI¥#?²hÂÁ®"@?jÕy§?~Âs]?°CIåšæÝ?°Ù==Z?ï"ä]]/?˜xþ°s‹?U¬ÿ:r¶?dÖràY}?šH¼4`³?—=b<-»K?햨jŸèô?"ä§èŸù?r,À__A?ar×™0Û?²'ð¥
ÄW?"+Øÿ™¶ë?ì'Õc]Šš?Ÿ†)á
H?zÊÆÇD#P?pæŒêp,?¹Ä¨xŸhý?Ÿè݊œ44FGL J0415.2-5741¿ÙošÑ–ÏÕÀEŸaܓê-À<1 'EÀÀ=Gýœ@#`ãÍDkë?¤=Æ_u;?ä':l˜•?ïüšò?ÿÛÄ?þ©úE+¿ïþæ?d™Þ?î¹NjÇ7¿Ë©nù²Þå¿ç8Ð@Ô?¤0Q<Ľ›?Å¿ˆÁ…AGNbcu1RXS J041505.7-574237?î
6hʙ*?²ÜmòžÞ?'w°P}?…¿Ôc×ò?ªÖ»‡/<?²çÐÕÇç?îy.£M?µ¸€¿ûw2?}
û´>f?'¢ìsтä?«'&Ž
­?´ã>";ù?ê´_Öª³p?¦Ê"¦ÅC?¨üßPáŽ?˜Ûƒ­Ž?½Þ'¢9Ý>?¡AÄãSO?åáÚLìÛ?Ãzî=Ék÷?HÎ8ʱR‡?]ýIŠíÊÅ?Ô/äKd͟?Ãz:X•ÞÛ4FGL J0416.0-4743¿ï´|è3IÀF½#N¹¡wÀ;fÞõÄ<ÛÀ<ßùË2˜Ú@Nšþsì@xä$Ø&?Ò-úNw\?Ë!É(}w¥?ø[Ƶ[—@(¦h´õ@?ïù–Ys8ݿތ¨ðN²¿ç›Ê`áÂ'¿á±§­Y¿ïÿ¯Èe_¿ëý€Ú†AGNbcuPMN J0415-4737?ïÖ&Ï$I²?rY^·5E?L>ñhR$?HO*3;à?qdºKN¾?p†Ñ«}î?î❍.?›©|7GV¼?b'ÐÄý?pqìŽóÛ? ¼Û‰ìä?™¼ÅŠ¯?î."ƒÒ.ê?'
©Á`?ƒ†(» Å?vé¢qMOá?¨67¸®)3?ŽØ µDm?ïmPT[@?PÔõ³J?pn¶J?_¡¬õî?™–Ô‡â£?€50ST4FGL J0416.0-6628¿ëœãˆÚÀCí½Q.ƽÀ;C¤as¸À<»ŸÖÊ|@òs\æ`@Gý'w>%?Â;…èí¿«£~€Ž†?ëIA'¼Á@º•'LC%?ï–T€4éñ¢Íõ¿硑J?¿3¿Ý½"ÅÌþK¿â&¦'¦`Q¿Ô´AGNbcuPMN J0416-6629?ïfŽ†6å?ˆoÛ0}ì?]ØFÁð³å?Qƒ1¦ô?'`IÃ(?‡zvÓöù?îìÞÿ´ÓX?™·¨Œð?X7zÛ?gµV'ÝK
? m¦Kæùµ?˜³D_ì?íâœGÍe*?'Wê"Rí?uÕ¶l"w!?f¥šÐ¨2?¯"µ—>x?'oÍwvÎb?îZlÚ¤­?i£€K?j')…?[ðXÇÉz?¨°T}Í?à8"ªµ4FGL J0416.2-4353¿âď&ÜÀFðîcŠ	À:ßÇÏ7
XÀ<žÑ0ߛÜ@rØòõÖ[@Ð<eáÜ)?ÆH3
‡¶?¿pQ¡³C?óÖރ®uÊ@a"²VÔοïÿÃ.¾Ym?ïþ­ŸàÛx¿æQìAZ¿ë3^ ò"Ü¿ç"¢^º¡¿ïÿס<%JAGNfsrq3FGL J0415.7-4351SUMSS J041613-435057?ïò°Ú,f?eڕ‡¾¬
?,I-Aá	?+ç¶øœƒ¹?Xnµ%þö?d÷_禂³?ï¤àY¿"ö?‰²
r? ]?:æ;«,|ï?Us˜Ìty?…ð·²Å^É?ˆ¡ë™=ÙL?îÏóYè?ˆÍ͙Èê?wV#y4Á?t3ã:? ú}8#?…ÁäºZw{?ïÍì÷Cçê?b¦¡vœì2?OíЏúšt?Dý'ÁÃ_\?uÊL·y?`Ô\]«Ê
4FGL J0416.5-1852?è'ù2öWÀE3§Å¬À9wc(ÄDhÀ<[²h!@†Ì<Ùû	@ö Ä0F?«ˆ>®ïö?¢ä,å¼1õ?óõãFŒ@Ge€¸L7?Ã_چç¿ãuÒêóÿ¿æ"	\ ¿æ'ä¾®&¿â‡vfœí¿åm¹ Èw~AGNfsrq3FGL J0416.6-1850PKS 0414-189?ïКتñ?t_Þ,ÍÚ?2"®£m9\?%Ç…Äûí?vis´?tÌsÄ?ïÓÝTë™?|;–i°w?"Ùë2"
?@uð'ÈG?uz¯|؟ô?zòP¹¼9?ï*–ÁâZ?ƒ³d",÷©?fªü¬Ý?T‡º­®8+?—×È.ê?'Æ©©h¤D?ïúPf½Ih?4æI>õøè?ã]²Á 6?ó¯wœ?CÁùT'-K?3YsKS¢ƒ4FGL J0416.9+0105¿ït—Ò<èÀ@"¢ƒM&úÀ9¦¾r–öQÀ<	¹07Ö0@ rÞÎ,j?þ4rHø"?±en™»¨b¿†:A"ÖJ?×]_A. @		l¥Å¡à¿ÛüÑö®H¿ä¸u\£o¿âkIYæ%c¿Õ՞Bà¿áÔM"ÞHö¿Ë¢‰pîUAGNbll3FGL J0416.8+01041ES 0414+009?ïÝ°mlhì?‰u*
T?/öjú˜˜?9²Vqy•?p/™–s´º?ˆRk£ïF?ïšy¸ûRà?‡ÐaOž0Ò?3‡ɧ]=?NžJÖj?ˆÅYÞ
]?†é7L½BÏ?îùŒCþ?"ÑO9z=?dÚÝ^1,q?TsÜ…m?žB2БZš?ƒü8È"!ä?"ô´Ù?ŒÈ_ǸC¦?^‰G—U*?N|tÛ)Ȓ?¦àOw÷À?Œ*ýøUÝ'4FGL J0418.1-0252?Ò¥†Þg:2ÀA…
¢q›À9Áíûñ}†À;ùôñ¯e@FÔ¸~Œ"@(N?þó'?¹5T`)‹j?ÈOFúTv@
d8Š‹	@™—‹wlô?ïÿ >ybm¿á¥ø¸
"'¿ãm9ßtÅ$¿ãéíÚcŽE¿ìo>±ìv¶¿ïþ–]úÝAGNbcu3FGL J0418.0-0251PKS B0415-029?ï³!SÐE±?|e9y0¦ý?iƒÌõUÙ?dNL4ŠÆ=?y­o[üÀ?vê{¯_?ï«Ùî¡Z?ƒ³¼šçe?8cQöÔîî?K"·2xéî?"FiÇòÓ(?ƒZ×½²v?í'÷ƒ*üM?Ÿú®ï?ù?¤ÅNB_Ð?—x—© û?¨»9Šðk?ïOy²…`?ïtØÊÀF?ttåa{?WEªFZ:?E[ǃ<ã?á#1-?sH;å±!4FGL J0418.2+3807¿ÉL,È,vÀ!ˆr)é–À8ôÅÕaÆÄÀ;mW…!@þ®ð}@ä_á'p?µæÈÌbÏ?Ã11{M(R@SƒãNïQ@
j‡ðú©¿Ó7ØßT¹Á¿äÒ3ß*b¿é¡ÝÀý¿è>°	G§^¿ëØÔ½‡	Ÿ¿ïüøÿZ¾'AGNrdg3FGL J0418.5+3813c3C 111?îsC‹|¿?¡š¯òÆ?x‡}³t:?u¾DÚ6Fþ?¥º×W1Ņ?Ÿ.f›}"?ì&ÔÅó‹?Àf
ßH[?nD|ÎXl?'KõO›.?½×5éðâ{?À#åÃåé>?íI'j_Ñý?¡]ºÛA?"µþ†c§?Œùý²Þ?°…ía)?›fX_Ð@?íÆÅÕ*R?•pe=ÄÜ?†×0=͎ï?q«dJ҅?­Ý֝ìg"?"¿*"×4FGL J0418.4+3414?ß¿"¢ÎemÀ&õû"‰µ À:¶XÆj²üÀ<-+œeü´@¥4°¶Áž@yõÅšç?Ò»ua€ùe?Ê¡õHAe?ö	Œ³?ó9
}‡jB¿Ã>ü•t¿íà
¹(*¿´ZŽýðlu¿àÚ&½+.¿ïÿÜßi‡ƒ?å;
óÊAGNbcu3FGL J0418.2+3412GB6 J0418+3411?èðП¸†?ÇŦ?ŒYMß?;Ò?‰DԐxBˆ?;§ß*)?ƲJ«$	Z?äuËÊ2ñ?Δ¨¢…q?Ûòø׋s?–«çú™ø?Ö%äФÝÀ?Î!ªÆlˆ?é-ó¶wÒ?ª*
ƒY?§†´ã¾4?"·ïy4Ë?ń×í1.?¦J¿Ÿ3?æ7Lû_ï›?²]ýŸ.´?"ja—ÖQÞ?†&òjŠ]?ÒJ¿ï»«?±ÙqEݺ4FGL J0420.0+0805¿î)ǁ*ÚAÀ<sz€Ïž8À:¬[y£Z
À<e|[›1@‹¨ÉR9@rT`ªdÃ?Å}
—³f¿"9r½aÊË?Ê·û–ã\@
Ðδ®rð¿ÝN'}ÁKå¿ã:}¿ÉY%¿ëˆ:̄¨q¿áåuoî¥e¿âàØóK½¿ïÿùµc#¼AGNbcuPMN J0419+0804?ïíjÓ/û³?Z2?'ŒHä?0¯óY¤?*±[À{é?`.mYß?X"ŽªÉ!»?LOâÏ?‰têˊÙd?5/£!µ®ü?RTÏIG?ˆlïÒùž€?ˆU~œ§&Ó?Ð/?'6­
O°?o¡¡­TO?a.É|	'?¥µlâÍ7É?'rƒœîÿI?ïbŠì"=N?xÁŒvE ?9HÓ¾Y›?,zˆ²|ß_?"HmL)\à?xo‰"14FGL J0420.2+4012¿ï™iqøY²Àf'ëØ+À:=k¥jˆ4À<q¾‰=+@!	'Oæ?ýHÊ#¥ ¶?ÃwA)@?¸NÇ~¹ï?ôòôcê‹$@ÒÛðX•?ïë³ýÈî¿ç Çä¡Ö?Ípž"ÀI¿ÞÔna‡"n¿Ú] #÷V
¿à‰äð°AGNbllB3 0416+400?àU Ñ@D?Ãæ¥8$š¡?p•Eê¸õ&?a‹ŠEM¢?ߌ¦²›¥?Ã璘ÿ¶¾?Û{Ö?Ä#\O¤N°?f1Ùu¯?u¥ò%ɲ?â^îÁèýf?ÄC{fù?çB]š¾Áö?©@RÜÐQE?'Úw‡D±?{‹é×vâ?ÐMR39?¨
-"³ˆ'?çj"ªGX¾?¨oæêÅ|
?ˆg8Š%{#?wYf##p?Ðg¼ç "¬?¨nìð‡æ4FGL J0420.3-6016?à$—óëäYÀDäÁ¨¬\À:ï¨NhBßÀ<Ҝ¡‹Öb@ãü>Ty@Stÿ†]}?ÀíS*Œˆ¿ŸWÐýD0?ޜš·På@¬ƒ!Ýö@?ïÇËLp¿åvÀ4ü¿å¤)	ä…P¿×",<žìÀ¿Ý@IQë¿á¸I©ƒòAGNbll3FGL J0420.4-60131RXS J042012.8-601446?ï¼,O5©
?v~û,Ɍ?E¸ Ã‰®~?7EVƒ&?2ÄLºCl?v
†Ì#¢<?ï¦ì®j!?ƒ%Y¡H?,øÌpÞQy?A>!õtµÉ?…Ðñ3¸¾R?'Ç'N'o*?î³Zao5H?ˆ˜q
Ýà]?iç;¶}?SÉ:S±ƒ?£9o8ð?‡q¸±J-Ñ?阮Ӏ•>?k¤4à–s?QËUCBF?@mJO7¿?ƒäêµ2H;?kOS2ÐÑ÷4FGL J0420.3-3745¿~šã*86ÀFŸ}At>–À9?q/EÀ<Õ]•@º–rȟl@b:îéW?­6(ÛìOt?¯
nݝn?þr!+û1@ ³0C"ª¿Ù€ÉS›ˆ‡¿â/2ÝøÄ"¿ãêÅX.•¿âIáf6ì¿år{Gžû¿ç¸W)²€ñAGNbcu3FGL J0420.6-3742NVSS J042025-374443?ïۃôØ1z?f|òô©øò?*KÑÅ? mÀ&ó,V?qmÕŽ´?eþ'v_ëf?ïÀhÑrœ?'$¼Mð°?*¯X+¨!¼?B'ø\Ÿ!Ã?~êÐÕéq_?ƒ€ÌK+Ð?ïDÇæb?zD´!à3?eј(õ®º?P`·f{=?"Âôd}Å?xdF[˜<^?ïÖ7Ö/Ÿ?`é$
7ȹ?F"å$|§&?7D.Æ|9í?rxC áO?_.Û
–4FGL J0421.0-0752?æjô ‰ôqÀBsUïÝìÀ:š*
ðƒ‹À<*ºè@ä²hG'@äŠ=Ü¡?Èö¤Œ'É?°o炅¬?娑¹ÑG†?ðõž,Á?ïý
Ú7¿æä¶Ê,	¿å §ªÔT¿êƒÈaƒ'½¿×8À¦MÝ¿ïü÷™Ã
AGNbcuPKS 0418-079?î£+B"?¬Ò@Ùˆ?iw}ƒ@?l3 XŽ#?¬¾\O[u²?¬7ÇüP$?íS5è"w"?°˜¸¬?ˆŠ¹Ì?")sÎ>§¢?²U
8Cl±?¬!×?ì^>‰êŒ‹?ž$v[Œq¾?˜Š¤f¤?'¨BŒ¹$Q?¸ç釁÷?š2<‡´?瓹¸êO)?«¡Ö,½x?œÇÓLZ?…˜"'Ý=?ι¶¹Ð?«˜ýT|4FGL J0422.1-0644?î´–­^¦ÀBäâmHÀ8Ïk=e¼À;ØyªæÈ÷@mHS*õL@¬¾9Œ?¦-º<@;ô?´ÿ+Ä©èœ@	†Eÿ¾'@¨=?üoR¿ÒÔÂ$'Q©¿âýÄMc`¿çpÄÜ=ƒ¿ç.³Ý¾n¿éÚ¡oB¿ïÞfÝڑ1AGNfsrq3FGL J0422.1-0642PMN J0422-0643?ïîû·#?Z3Æ1&?9Š?(¯?25'›|Ý?[È1)?Wùí±°ô?ïÌPACï?{¹áÉ~™?07Wo?F)Ánæ%?xÔmåó
?z®
‹q?ï'ÊçYdb?'äz>"éå?pþïyùö,?c.¤ÐýÚC?–Æç6TöA?€ë8DuòÅ?ïöàùÌBè?@õw¹½?"\ó4Àþ?Rµäbi?OúA''0[??¢å8î]ó4FGL J0422.3+1951?ïÛ=#)®XÀ4œ!ÄuæÀ9òQ~wÕ$À<2¯È@ 5;K/©@m|:
B?¹Ç¿FÒLi?‡ Éû"?ÑÝVlGQ@0fšhÌr?ïÁ¢a¿7¹¿çöÿ.=*¿â Va¶~W¿ÕApx8 ¿çÑ@>ßcӿɤCZÃÆAGNbllMS 0419.3+1943?ïÞÿ>À{?|Gò†>‰5?7Á	¿0x?/©yåã
?nIÝË?|xZNåß?ï²#/e&?ƒ¯f"Å*Q?4¼k°†d?G>xM‡…Ÿ?'ÙÖ É24?ƒ=3äˋ?î¦Tn"=?EҙÜÃ?nXò.Ê£?^"Š¡'Y??£µ)öÉ;_?ŽVw6>ŒM?îQA_›u?‡ãw
P\%?rÆuÜø>?\ëéy¼$6?¨"-[J©²?‡ <Ÿ>Ö4FGL J0422.8+0225¿ïœ'üAY'À?.¢ ©XSÀ:?Ã<*RºÀ;óvñÎäÕ@–7t‹m1@
'¼«ì?ÎÍÉaˆ[.?äN.Km@ Êƒ@¬Lfn¿ÌmÆWߦ¿á(qy‹¿ì!yÍKwοïø˜'˜K;¿ìl5恿ï¦Ñ€ìAGNfsrq1FGL J0422.1+0211PKS 0420+022?ìÿ'`‰'?¸{kI~?¬µ>èQ$?ª
\7»?±=dŽ2?±¿WÙ‰?æ|ŠºŠ?Åú¿!H*Ä?Â;2Ehã?Á`c«G®0?ÅßÒ¥?¬ô?¸¯lcÞ1?åח(ûë?°µ™Tô©³?À=K^
?¦–fA˜€°?ÈdX¡òK?§­†`i?â
&-e?±¦£Ž?¾þ›Ìž¼?£¿\òâ?Ô,:Àû½‰?®¶F=â4FGL J0423.1+2106?æ¶L:@B»À3§ÑEØQeÀ9É2ÄxjuÀ;鞍õ ©@ŽÅ9°zÝ@#¿!é_?»Jm·hŒ†?³ôÓ|vÕ?ùÝÑ6¾Øî?úO–@HÅ¿Ø¥bïڿهã¤)Àn¿çù‹!0Ò0¿ß8÷b¢Œ‡¿å·a¿ðAGNbcuTXS 0420+210?îïÕ±.Ã?"¿Ú):¶?x
ó¯îÛ?p.ŒMÜ®£?œÌîx‹Ä?'T¤M–WB?í…?niY?±ç¬jÁO?–ocqå'Y?ž&@Ñ®p?±ÿý(PÜ?ªö‰OFU?éÅ0ì—xH?¨óÄ↮W? ~'7NÂ7?Šá'{e?Ä˗ÿÎnS?¥¶¡?ìF?æbj†–Úì?¨7øÍÐWâ?²? CØ·?– '«]"?ÍVÍU'§ò?¥ƒ¦b=V4FGL J0423.3-0120?ëð\aC¬À@>}QÀ8
g†!ÑÀ;Á%ϝb@•,]@ätÙÆ°S?ÆÅÝÖp¡?¶˜W¾òˆb@ôaùð†@uÏ¢<x¿Ó;ž̬¿àO8añ6¹¿å-F¿×ñÄ¿åâ;Ÿh¿çèµ@i&µ¿ìsüPHAGNFSRQ3FGL J0423.2-0119PKS 0420-01?ï¼håi7s?vä`ÏR?CíOâHza?fHk²mrs?MãO7 ?tH³å9"?ï·Õ켸Ø?'ùóB˜ÇF?:ÂVˆÄì0?LÊ
.£?4r‹¢Š?'£oïêEÛ?ïi@ã"j?}YÊ)—ï
?q¶O+À?oöd6qäd?ŒÔÃ1·O`?uwšIû!?ïöU»j—
?FB$?U¨?pb÷¨?´F;•P¨?Q'ûa‰?Ex©0+»«4FGL J0423.9+4150¿ëÊ÷nN{À‰äÁ¶UÀ8X-'JTÀ;`e':ØC@¯L$›À»?üƒ3á®Ü!?¥–˜Þ2и?»övÿ»·|@Áv¹Ã@¿úQo¤¿Ì«¥'[¿ÚÓ³¼¨†¿Ú²!$袿ÔïÂ',j¿â"n!EÊå¿ãÛG¹ÒõAGNbll3FGL J0423.8+41504C +41.11?Öx8Ïëe,?½®épÒ?£ŸöFgð?š³Â?ã"y˜¥æë?¾¼˜ŽâB?̚üÛ½J?ÇêøáæM?ÆÑì6Ü?ÆQV¯3Á1?ã$ÅÇÊ_¥?ÊZ<–œ¸G?ܪ²›R?³'Ɉ"±W?¹¶]"/?¡Íê9v$?Ý`Q¢>?²úž'Vˆ?Ôb,â2/?±,ÑàÒÔ·?Áp*èø?¨r1¼¹ê»?ቩrò,«?¶[碡Ž4FGL J0424.7+0036?׌)ù"À?ÆñVIÀ8«ü†Î»ºÀ;Ý[o'_@Âqû@JTFŸ?§£aÍ/?¬îÄ$÷J@瀕Ó;@S¬½¿œ¿×Õi>!²¿ÚäÑ@±¡¿ä…péP'¿áäø¨ê¿æFV[Vgì¿æÖlÞ¥'KAGNbll3FGL J0424.7+0035PKS 0422+00?ï¡·eœÌ?|ƒ¶wm'?C+?–Œ@q?:õQsŸA:?†_rŸd4þ?{å+ӈ}F?3¤•?imŽÑ®?M"iÝ/?a÷´~ÀÈ?Œê÷¹
d?‹i¡"J‡?ï‹ ù–?‡žlä fQ?qäøu›ß?k_HÍõ½í?šÕ]áùÕK?"¹íÅÿ‡?ïg•6(?{xRÝo‰›?rW{§?c|_L…W™?†Â7¨°?u¬Ë+r †4FGL J0424.9-5331¿À¦\m
¼¿ÀEÓEŒÒÀ9­ß…65FÀ<A»±–^@Ź'Fî@"
f‹OT?±®xßöÜQ?½U&^Iȇ@
ÚXÁb5@×Õ?7"¿—I›ªjø¿ß,>ø8`¿ã+åï¿ã0AFmD¿ê¤E>Îqè¿ïþú|2€†AGNbll3FGL J0425.0-5331PMN J0425-5331?ï¿[,Üþ?uTØîM­í?RÄ£"(?Jbò¹²Ù?{¿©¡P¹?sö˜Bh_?ï¬É¢W—%?ƒº
.ŠTb?9ùƒOC'd?Q†¥Iƒ?ƒýËO Ô?'Ä@ƒÐr½?îãúØžz?ŽFøÝu´ž?ƒ¿ù:Ü—?'ÆtK¸ž?™ ¨`>!‹?ƒ—bؼžå?ïÁQ¶1 ?b#ªSzí?Q UØtˆ?@;œ©†ï?{#qQë?`!]"hK4FGL J0425.3+6319?ïÐrÊf°@#‰ù&ÇêæÀ9ì
±™kÀ< ÌàîÂÁ@!¹ññIƒØ?ý_ñ7n+?º ³iNx3?"êxg«ò?Ø©ßAÄpˆ@ò`gžÊ±¿Ùž´@cóE¿å®Å"T¹¿ç¼=s(¿Ñ÷†^ÔKÇ¿Ó\ž¼n¿ÚæØ;ÀËbAGNbcu3FGL J0425.2+6319NVSS J042524+632005?ê<ÄÈöJä?¾"\	´â•?yÊ/Ü$~æ?¬ËøM_ ç?Æ>›]E°z?¼ b'†9Í?ä­^qÉäÍ?Í©¨óÏ?s˜cI€Õ?‡E9šÁ™ ?ÖVâÂßb?ÌÁ±¤³Q?é¬Ø`Y»?©O€V÷«?ŒÈHWí¶u?ufÉíìZ?ɼÈÿ½­?§þ¹˜óªØ?ë´ 
æÐ?¤Áȑ¬?ˆw¯'©xš?|ÛL»[R?¿P	¸tP?¤%TèêE4FGL J0426.7+6826¿èˆ€•ìÄ@*º=ú	FÀ9¹ÏµqfÀ<6¸©õ@!lµàÍ
@˜vƒêÛ¬?³¶ûª0?ª´Áp'ý?÷³{?D@yáSígø?ï÷ó¡Íś¿à³ŸÕý¿åŸ+ÿ¸1Š¿à! Ï¨¿ãPW›ÈH¿æ]4Ž}åAGNbcu3FGL J0426.3+68274C +68.05?îäÊ ùù¦?–£6²ý?eQe"7´?Z×%•é<C? ^Gž7' ?•emS%õ+?eوþ?ªDgá~Ê?jo´šFÊD?
‹"µ­?¦XÆ?©*¬Åçt?îubÚË"?¨¹âoÿG?uÜT†ƒè?dÝXº{.~?¥îGÍòÐè?Žõ¼[û?íZ•¦¸þ?'\e°>ã?™"ÇGpT/?|tÓHÉw?­Ì³ÜEý?Žzík@î4FGL J0427.3-3900¿îÖ¡a[‡ÀE÷—$tSÀ8ä01öóÀ;´bTˆîQ@å†Tmj'@¾–ÃüC³?¨Î½š
L?y~þÈ#n?ʽì(2@xS/'
¿ÝՂ}ô!¥¿åÝÓð­|¥¿êœ¾™XV¿ç8®6Ý¿ïüC²\´?ï|.NÇä0AGNbcu3FGL J0427.3-3900PMN J0427-3900?ïùœ9þ[Ä?H1S¾p)Š?6±ƒ%t‡ ?7Ê9´{R?<l¬ç­Z‡?B)µz1µ?ï‹cÉw?•­n-¤É?NUøñ¼†Ô?pÍ[Ì?‹A®*DY–?'£ö,Õø?îfqN?n?•õâºìÁ?ƒ8J•Ï`v?x' ó?¤ÊØv•>"?'@M0|"b?ﶤ#sÒ?s¬;tÙÙ?\쑋3âå?UsÎJEw5?}rÉã©¿?pØÂ9£Ÿ·4FGL J0428.6-3756¿×¦\š#œÀEέÙ©TÀ6EXôÛöÀ:©fã@È{zIÈ ?ÿë|Öt+?†Nӑ{׬?´ég,ù³@*Lˆ3?È@ QúÖ `2¿³¢ðŸ(¾¿Ú#¡ZX;*¿â'°âÄ¿áýˆV{7¿åé`F'µ¿è Fý"5AGNbll3FGL J0428.6-3756PKS 0426-380?îÙ¡°(µ¨?"˜pËa7j?W3vö,Ck?X6?¨)?¡¬IEÃCf?"L|§¡a?îi±-Wð?®±€_ä\?x<Îy1/?"¹ðœÿ?£!Ë`S?«Ùþ6‡k?í>~ž†è?¥B=¡ØU/?•!ØL•Ç}?'Zøk2?°Ã"øª†Ù?¢^ûv>1'?îÌ¡áˆ?šW§üp?j×6¢½"?m˽* Êg?¡ˆ|$fb?˜Ý¿sª6w4FGL J0428.7-5003?ï<)scFnÀE‡0HAÀ;O¥^ɹóÀ<ˍg\/¬@í
¡~?v@"!4x®?Î×^v-í?¼/'(áö?îŠÒŒ)nŽ?ô†ùç71E?ïþ±ëÕ¿Ò''Û'‡¿èˆ¥@ï«¿ß'£G˜E¿ïÿŽñ ¿îxê݃ÿ)AGNbcuPMN J0428-5005?ïÙ¾Øÿô ?pÚ^GÈv??ûr;é?UéÜ£jË?q("Èå;ë?ow‹dñÝ?í¶ng?¬K±'w"–?ƒŽcÉS?'(Q<Ü΁?¯º•&×~?§þƙ«0?íH\ù¤K?—·£bA²? ÂÙÌ4?Æ~Éês?±Éßw¤?"¨å»¦´h?ìüºîêà´?™k·±¬º?£)jÔ¿5*?'Ruƒ÷K?­
æ<'¿ ?È+Ï¡ôÌ4FGL J0429.3-3238?áh$¬ÀEzšu%FÀ;G\WìÀ<иãá¼H@P¦?p?ý™¨bŠ8Ô?ÏN×(›T°?Éó˜Ôw¼?ö1ƒ/ÊÉ@_u†iç¿ïü.ÿò¾ú?ïÿërªAˆ¿Ú#|"jÞ¿åÀ¾/@¿ÒéûF\Û£¿é*°bˆá;AGNbllNVSS J042900-323638?ïŠÕzy^­?€9´í¸KI?V¦ýCÎ;?O7XS™#?ŠuÝ¡ÿÛ?~àŒÞ&¾?ïL$."Û?âáþyU?L±Ile?[cI€>¾?••î3<h?Ž£ë	Ã(˜?í¾Ý'Zb«?'X¨†Å,–?…ö
JŸ ?ys‰¿X&?®"ª÷²
Z?Žðä[¸ô?îûpÕñ¤›?'ÔŠì°Ù>?d±Sæy?Y®Ïóõõ?ûºÐe?'Kë§4FGL J0429.3-4326¿ï¾û¾°]ÀEÅõ@‰]À;å(
eCÀ<¶ýwÞ@bå®pg@ýø8‹?Åê•_£(º?¨ "ûé¬?àÿG¾…ŒF@:~6Ë¿Ú&Gݏ<É?¡9À–¾»¿å§ûâd
Ç¿ìSå1[¿âWÝó»¤?º‹¤ùÜAGNfsrqPKS 0427-435?îڏsðz?š"®•@—M?SOÚÃ(ýK?IÙXØgË?¡Ä˜2§°p?™Ùóý"ã±?ï0}CÀÜ8?"ñ?Ý47?Q>±ÅfÇÔ?caw´?˜ÜlkŽ§?"è^f¿Ö?í¥ìv|"?"'ìÐ2Е?"ëåõ]M?vž¸zŒ?°LþÓ5o¯?'y(‹C?ïq3Ô—_?w"ì)'ó•?Uµ\³êò?HnÍEH…Y?~/±Ü%;?wD‡ò|ù<4FGL J0429.8+2843?êi5úäÀ*óÝüŸù/À9RîؐOnÀ;ÃD°E®@½?Çk9	@` ßs˜~?·‰Hh¤"?¾Ìևá‹K@¢õ:ªú@5PQQ+l?å$Ã9¦¿g¤Ò»VáA¿áhçv¯Š¿ÛuÓáéêj¿äï ×{|x¿è	çàN‰ÑAGNbcu3FGL J0429.8+2843MG2 J042948+2843?íã$ï‰?».ã(?¢-ƒêqæ;?»'Ü܉ÕÌ?¬"KS?!A? yÈ©€¬?삓7S?·ëÛÒkNÅ?¤mUsÀ{‹?¬Šyy-(?±´»Š)›?°™¯3¯×?é®ë=‰c?©"'†&Xý?ñ°gY?1?‰8ùËÒ§ª?ņþú²Š?¦ëæ¹?ãÝÅSïò²?£3Dä?¾çµi§Å'?›•)€/G?Њ‡ý¶)R? "Ävj‹4FGL J0429.9-3101?ÚpÃÜÀEIË>WS¤À:&˜Û-¸ À<r$ëqÔ@!uƁ?ýJ½"så«?½¾¦Š˜Ë?»×xÍFD]?þv‰Ê½f@Ô:®0?ËÍ2xMC«¿Þ¦^c™¿Þí,¾¤ëÝ¿ÓPNâf<¿äò?£%¿ç´v)RáAGNbcu3FGL J0430.1-3103MRSS 421-156568?ï}Aì£VÞ?~zÇzE-?Rhf'ª™?EË/ù©¥d?ŽbxÕÿ?}‹[a¿ä¤?ïlÒ2œí?Žª²uÜVÝ?I†På®À?Y0õ"J«?'…{Å5?ŒÔÚÆט'?îV5ŀܶ?ŽU>]" ‡?t©‡V §?`ö¨a­m=?¨r½1g?ŒgÎä†?î×"»Áuª?{êKõhË?r9}à¸æW?YƒÖW
? F¤‡Ñˆt?yœ¬‡Üs4FGL J0430.2-0356¿Üˆ¨^óWÀ@}7\ŸÀ:ÖöV3|À<i²?'ÌÎ@'¥e՜Õ@øá…Áu?ÐRVy‰XÚ?º¹»£К?ä¤Váä-@	ÓÆë|5¿ÐbH_bŽ¿æ(ºžÌßA¿è,PÓ¿î,ma,j¿Ð|T¤Çõø¿ïm í¶QAGNbcuPMN J0431-0406?ïäÏTµùç?n}A1€i?$,¨G!ŠM?*ZÖp K}?iíàœÿ´?mÊg[ÇòÒ?ï28k#Õ?¤Ãšm¡qb?S0•%‡`'?on<HÅ
?˜…õàCT?¤¾	6d?îƒó<xÀ?Ž÷¼©»µ?kç
2D?e¸Ý|‹Ã?¦Z÷®pÇ?÷ µ¼4Ž?ïÀ¼žIç•?g—]c?';™FôŒ?!6
ñCˆ?~çÔԔ…?f×[!‰"4FGL J0430.3-2507¿ë\'YèÀDFÜ]cˆÀ:0%°"±"À<z"UŒúO@wàÎ'.@0ñ¤óið?¹^€hñ;?œf8n0Š6?ã5Õ¿º•"@¬7ñ³â?ïò+
0À¿ãî!	¿â¹·a*½C¿á;w¥S¿ÝXODù"¿ðAGNbll3FGL J0430.2-2508PMN J0430-2507?I»	
?ì™%Y^ô?Yz'oHÚú?RþÑæ•­?†aCT¡P?€j:€I26?îý@V4-?›'\–ƒt?Sáÿߺ?`5¤§
-?Ÿí¥G¬z?šÉƒïŠWˆ?ígJþ}ø?•Å}ñ.?‰?öädª£?{qŠhۍG?±©/ƒª
?")ô:ëÄ??î_StE#Y?ˆÓ¨ež"?³È]¬‹?kyd°x?¦O¹Ú?†©¥ôâÓU4FGL J0430.3+1654¿èÙɂóîWÀ5
ȁäq.À9—ˆŠ}œäÀ;ÉLíï\D@dƒÖcÏ]@Ŝ[cÔ?¶#Ú$ÏU?šƒX ¼3ß?ã¤Ô•îê.@ÆîÍӇý?ïý³õerK¿ƒ]$ԚĿæéu¿Ê°¾¿ãڛ!Y¿ãxê݃ÿ)¿ç}d¿È,AGNbcu3FGL J0430.5+1655MG1 J043022+1655?ï"F³E\?ƒ2J!ª?U™>¼Oái?N܊‰Žÿ?ˆ;+g$­%?'9,AéN?ïIA¶x7?‰€ÏûÑT¤?Cêä· â?PÙM,ß?‹oFð‰?ˆ}«´o#?îqWÎ}Ä?–ÐN÷+ck?€Vt€!!?q3ƞì?ªô"åø~?"¼âŸ¼žÇ?í[ÿxRöC?´\—Ú‰?…n\tq2?mIŸaT?²öqÙ¿Ì?Žús^tOó4FGL J0431.8+7403¿²íDkEǀ@1^‹\¿ôwÀ9ÿ¦å²vàÀ<oLjÀ-'@ýBÝ ?þë`ºU?´åV 9Šª?¥8iRÿ×;?ð£~õ©e@fuÜ{ ?ïÛS]u&¿×^Ÿ"¦¿ãû–yS¨õ¿ØaéÿãzŽ¿Ö•ǶãV¿èÜ)áû³AGNbll3FGL J0431.6+7403GB6 J0431+7403?ï֝•x?gRH'þN??
áèãø[?2,&6Òì?rÀ‡Rµ²É?fù–8á"?ï·^eÌïÊ?½-1SÓ²?;jB.Rùø?OX‡…H?M{Quý?€êœ	g?ï;†p ?ƒ™_&QÞ?f‰è븯.?S̓폟-?œýqºæ'?'ìnŒç·ã?ïhcõÃ3?tyôNõ,H?gb'ÌáË?Sp;ÛÉ©?<ýw?s¸ïˆ\â4FGL J0432.0+1732¿í5kÈ·$«À4U.ÓÀ:ÆYåN£ÒÀ<pz¼^À@îQ†…j¹@Á]¥Í"ƒ?Ô'øR¸?Ûß©~+V@µ;ÑgfA@"pµßö? S~œÅ¿å(Уñâ0¿ÜÚsÿV6î¿çLê"]ðv¿ï»batE¿ë¥­Aí
AGNbcuTXS 0429+174?é}OˆÏ'?¼óõŽýâÿ?­AB¦ð-À?¨¼Ç'2G•?Äqº ¶L?¸•f?ìuƒõ=?¶`ÖŤv?šŠ˜¨G2ž?¥Jñ©79A?µ±=ÆDK?±ì\BµP²?èdÚ5h?«	yÝ5I?µ§	/Y³†?n¼Ï´óE?Ù"ð?¢¯Î*•j¡?â4mW™E?­…gF?–¹Z]?ƒäâ7µC?Ú+/ƒ»ÿ?­`¸âdý4FGL J0433.0+0522¿ÑhžFsúÀ;j¡è´lÀ8ôxmÏç4À;œ=þhP@4@§ºï€@st¼j~ú?²‰`
0ë?Ðý ¿¨¡õ@×õûn@…¤Q¦ù¿×›X¶z{¿ãìÓu]¿éÏ^âäfG¿ìª$Ìh"ÿ¿ð?ëí×^v-AGNRDG3C 120?ï£m#ÝQÊ?"ËßØ'çk?y8e7?|j=å·6*?u~~žµ»?vŒ@êá 	?ïv™ù}9û?˜ÚSzq‹è?ZÀw2¦¯Æ?vn©AöѪ?rº\«"?•i-º6)ý?é™Ôáué?­ë*ïFA"?¹|÷}Îí?¤
V<ì?¹µQüÒè?£†‰!¡¤«?ï‡FËÞ4Š?|èA6è?\Ñf#á¤?R¡Zi¯?Š" GÎa™?zÖº…Kã4FGL J0433.1+3227¿È"°êv´pÀ$åi+<ĬÀ:7®_ú;›À<(<üàÏ@!A¯à+#?ýhò	1?ÂP?§¿!?¥Ùr€-À`?ãn;¢BŠ"@ˆ™úg±?ïìŸ/ۏ޿ê.8!¯}1¿á¥îaG¿؟Úép¿Ö
µ%;Mß¿ç› Yý!AGNbll3FGL J0433.1+3228NVSS J043307+322840?å¹VqcE?ÃEh°»?B?iÕ³ËPƒt?[AŸÃÃ?ÔY§µ¢Ôè?Ã>I1Ç?ç²f…Uo$?ÅÈY÷è?['•JXÚ?kãÞúhL?Р`
ɤ?ŵԺ©
~?êHõ
);h?¨Þw=v?‡ç~!ß?q-NKë-?ÅkýSr D?§Å°ó˜(Ø?꾊Œª2Ö? Xµ©Æ?|­ATú+?kUQ#Gúò?Ä msLŒÕ? šéš(½4FGL J0433.5-1039?è÷`\C«ÀA²÷üü?À;vºq€vÀ<˜Fíû¾@éEÔJ›@'µÿ_Ç?ÈÒ»y=X¦?®ßM>2{ä?àˆµENJn?ü\±+†–ˆ?ë.-9ôîT?ç­½"4Þ.¿ã&ä¦f&¿ãñV^ÜY]¿ïòbRÛo'?ïGÿ¨Â+‰AGNbcu1RXS J043333.5-104220?ׯÜ>?…9ñè/!§?g"§æé"?d»ºϝ¬?‰´`¶n?'é'±#2?î¯(ä76ë?žP:ò­?j=͆ž¨Û?s‡^mÄÏu?£i"ä"¦Ç?œê«ÑS?í0J˜dL?˜5dU"O?"Šë4¼q?"œob"R?±›''Ƅ?"_OV&¬?îK+ÇQ!¥?'&ë¥?ŽAQÄí¡
?Ì»ËâŸ?£¼ï²}T?Šþ.j¨U4FGL J0433.6-6030?èÜ
¬E1§ÀD5\ÙëÀ9Cº­˜#À<!.b@ݝ^ä'@¨— B•§?¨îL¤Ht8?À³l©v†@:x¯>F@¨Úã:øO¿Ëç*Üw¯¿Üp5½Q.Ç¿æM±>&p¿çÒÌ ×üV¿ê"—8w¿ïýÚV"K"AGNfsrq3FGL J0433.7-6028PKS 0432-606?ï²2dEy?wě㝬?h-Oþ´àã?c¡ç³­Ej?zÐ%ñ'Ó0?sN,±Ê#Å?勇"ÄÓ?"÷øu?žY?E[5ûBJ?duäa'k?"<Ãï'?ƒc8·%À?îÁü\ü̾?ï÷L/?"²‰ ü·?
ân¨‹L?gk›ÕéÌ?‹1˜Ñvá?ïÙeî|Õ?Z""@ä+?QsJ¢?µ?@«¨@VTâ?màl2ӊ ?V5!͎»¼4FGL J0433.6+2905?äzÓY?²À)3¤r:¯ÿÀ8\iñŽMÀ;9îיå@1ºv^;?ÿ²lHþv"?¨	Ê?eò?¶ÜÝæûw/@e^è¬@»G»ÖZj?ƞÅ''êN¿ÛnÂ@öö¿àobùÊ[Ù¿ßÄ-ÁÚ+¿ä!¸âÓõ¿ãH݉³r‰AGNbll3FGL J0433.6+2905MG2 J043337+2905?ïá¨lA¿‰?`s6¹º?De5¦Z,,?@p•\¢0?i>FT©íI?]7… MM?ïÄò6ØH}?‡'á_å
?9•gÍÂ?I˜GÉl+?{îËBÅD?‡VÔ±ßé±?îQå·<"?—ˆ31ÈcÝ?U.Պà7?zc¼B†Ý†?¦š•ï)…Ò?"ö›ÜoÌ?nÖ^Ï?ˆóRr¥h?bˆªÃK°P?N¨±â?¥ÍfeX?ˆšrŒàŠ4FGL J0433.7-5725¿ïӟJMÀDvŽÞT´À:Š:ÏߦÄÀ<š©glö£@_]³d?úBfýe
?Àé(M&#€?ÐC†g­Ó@àÇÀôQv@Sn9œ?ïèC ¾¦ï¿Çq¾ß#fŒ¿Án+ALP'¿Üɘ$y‡¿âw3"«C¿ës,è–VïAGNbcu3FGL J0434.0-5726SUMSS J043344-572613?î)Û oI´?¢_BY—$T?œÀ-]$Ï?–ÂC?YP?žnÖ¹¤½?•ÔfWl	©?íÞÖbäô?¯mOòÉú?|üę¾‹e?‰‰Çâmé†?®~Ê™ßh?«ƒÎ—ù©0?ë:3`*C?©´ëӋó?´ä÷Õº5%?¤;^ÿ<Ìù?³6Dx½?—9äò³M?ìâÜ4.m?™f§ÂŽB?†x»Z¶8\?v)¯«-ˆý?¶ó8e}?—þ	¶8éJ4FGL J0434.1-2014¿Þy^ðÀCzÞô¾À:>))ÄõhÀ<"VE†òÎ@&.iIð@4FY€¥?¾£eூº?ÆJL)y@f¨Þ°û@	éaþw¿ª¿ë¦œÒþ¿¼ÍfC½¿áLýpÇ¿éòB<»r1¿Ç^,»C¿ïÿùJYQAGNbll3FGL J0434.0-2010TXS 0431-203?ï¶<)Äs«?h°¤«?V¨t÷[ç‹?Y/Ïñÿ¥?7Íßï0'?|_á‰/?ïv>ùŠ&??¹«h]&?;¨‡'	g?JCŽÍ¡Œ"?É€pœïú?cm¨z"?î¤BA¯ZR?Œ)=*?Jªd ,?våý¾eQ'?¡Ò†˜Š&Ö?‡²µ!ÝÚ¥?>Å%?rÖÀ 49ê?RLM‡ß~H?Hpz…¤
%?‰Ò/RÇ/?qçšsC)í4FGL J0434.4-2342¿ãð*y?êÀCùáuÑ=À:{k*ñERÀ<ˆ]
ô@t/"î;@¼'Æ#?Â8MyZ‰ä?¸IàsȤŸ?óIxÔýó¶?ÿþGn(¨?Õ%‰&"Ï¿ã‡"ØaV¿æ·k;¸<ó¿ã6_mMá4¿æ:®â¬/¿ðAGNbll3FGL J0434.4-2341PMN J0434-2342?îZ¤Šâ‰? …"­Ð†?iG¬Z×ð?]!dz¶53?¨Á<˜ÄXe? 2lç}ô?îJÍl?§qXN?q»ñj³{þ?uº!PÝõ?­WÍ%×ù¸?¦k««½H?íÒ^ayð?'p¾¨?ƒgWž"…ð?rJtð¢r?®D¯¿‰?Ž²è…7?í¯'KètN?ŽÃâ]ú?'Ä
ñÞD/?w¾[¼J?¬+"H‰™	?‰ŸÙ;O4FGL J0434.7+0922? ‰KœVÀ8ñ|å-íÀ9—b=⹞À<ˆv[¦ð@ RGS?þ9¬CÀI1?¶¤u7d›?­-rð³*?ös?wåë@0»O÷º?îÄâÞ0¿ä/P…S'x¿Ø,¹¼¤¶ƒ¿Þ0{rçÿ¿Þ\ÐERD›¿áÜP=Z(•AGNbll3FGL J0434.6+0921TXS 0431+092?ïàAøíí?xôêŸ ?/$·¿:? M2Xe/?mË»¡–ñÜ?wéªË՟?ï¸:³á©?€÷6}'}?1½!¡q›[?B5#ífÈ?ciú´Ž?€paÉ	¸È?ï;Bð¨?'<'$²â·?h'Úg
ò?V2h¿nvÊ?›w+U	­?Bl8™_¼?î¹À7$°?kÇ{ô¶'?bÔ¨gì"?JìÁžn?£6»s1fD?€þl¿$y¡4FGL J0435.4-2623?êßÇÓóvÀD6ä:§›»À;OÞÉN"À<³fZOØ@¼{päš@!G®zá?Ê-ªɏV¿'³Í;Kta?Åû€ÿÄÆÄ@xsŒ>½*?ë¸[#*?îì1¡¸¡ó¿àµpà<ì¿æû½¥h¿Û¯ùWoRž¿åQ‹
ÜAGNbcu1RXS J043518.7-262120?ïŽâj?~Ù$â	ó?gÎ]AnÈÓ?`-fYèŠ?†‡ð#Í8?|Ô̶ŽU?ï†Îì	uÑ?‰ø¥Hl¢"?@ ÞjZ?Q2þZ"x?JD?»æ#?ˆôêY­ql?í®yîÖ±?"ÝITÞ?…š3ž»[?wš;åkÏw?¯±à·?'Qíhf
(?ïZP¨g'U?zî×ÌÏ©?dï‹hYæ%?]T©B/˜[?'ù†˜¬?y`^L€	4FGL J0436.2-0038¿Î)Ö'¿aªÀ>›Ã?…QÀ;«ÆÂǐÀ<¤Zk†`Ø@¯}óJå×?þ"þ)f*×?ÒZžý0ÂÁ?Üÿf<Ÿîr@êf}ãZ®@'§Dýàì?É»…õLô?܉uʇx/?Ë| 7 ¿ä',ëp¿æÌÁd8å¿ïöBmbÚAGNbcuNVSS J043614-003637?îUÿ±bX?¥¬Ê™Æs?ƒÖÍTza›?†Pî?¥ªQ"»ç©?¤/m"2†?î9é?ìÔ[?¦Í"<Ip"?vÄWa#|?…øáªè.‹?©ˆáÕé?£?Lê:k?ì'6R]ø?¡©X÷½êD?›¢ô®Ö?Š¬üÔlM?´f3DŽ?œכô­ ?íX¢
Tp†?"Fë«ïF?‹"Ìùû?zz·"…?±ÊVÙܓ?'™FÃ%ÓÞ4FGL J0436.7-7148?¼"éñºGÀAûÇ£˜ À:ÇĹ­À<‰‡¿}@ð¥¦Ã"Õ@úR¹á7¾?Ä1?¾
†?¡J=CŠø?ÜYÀ@Lv@¬ó±³?ïö!úü‹¿ãë½RÜF¿åòCŸ'Æ¿Û ë™á¿é\,9
ä¿ähF&*AGNbcuPKS 0437-719?î)2º©Þ?×QK"ô/?{'¸xsÊZ?'>&á³e?£›5ÅFèÕ?˜0Pà£þ?ïõk"´n?""!p²6?U£•Ý•Kê?`*ˆ´a?§/°ƒ?"¬ø°ÝWC?íåÚ朌?'•ëÕÞ

?{ú8;˜#ƒ?jò"ºr»?®#
ŽËrÌ?6÷…ZöË?î<Z@}ɝ?…ïHQïyá?'ËJ,f?i	yíԈÕ?§¸)%˜L¯?…)[cÍ6î4FGL J0436.8-5223¿ì;_&¬ÀDºëp&ÉÀ;x¶ËÈÀ<¤FvÜÖ@+}‹Q@Þ0å{|?Á҅ÉX#-¿³­FàH?ðÆB‰èK®@
¬Tš.‡¿åCªåx,¿ë‡—Ù¥ù#¿å>™=~:ÿãx^Kò¿ïy4i"P¿ïúâm©QAGNbcuAT20G J043652-521639?ïó£Ÿ3M?ZÆþñŒÄF?I?ÏEFz–?K™ÖÝö?Ja¢=ìY£?R°‹'?ïjÀÝàü0?'@Õøf!*?E÷…ª"mû?`è¸Sf?'ø(fÅ?r^p?ï ˆg#?…Ê*'å‰?gd¢lÎ?[{̛Û?™^Ùr¯?…¸YÛ¦r*?ïÁ¥÷.\f?kI6h3
¢?PW¹Ø̝?FQpÇN‡\?{'›šv?iV6Fb4FGL J0437.2-5846¿¸|8`0ѶÀDØ@žUÁÀ;:†—DÀ<—7£|g@ûy¹h@`V#ùŒ?ÇÝÌ#""z¿š¡éŸ@x?Ñõ몦?ý›Eìu?áŒwr¿ét ά Ý¿ìx¨B~՞¿È§ùÈ-¿éoîo´Ã¿ïü–ž½oãAGNbcuPKS 0435-587?ï' ²R?š"ºr)x?cݪÀv‰i?`mє™6?‡BôǵÈÕ?š ºpÍ/Î?îè+E*l?õÝöo?_=уo?o<ñØù|ô? ƒbæÓm³?œ*¹âŽö?íÀnj*C?"Òù׆±?`hÃep?o½Ӂã'?°†"}1t?'¾	iíÉr?îœPîÎÍ?Ðk$`?€)¦6zh­?t82­¨#)?¢0•ƒty?‹…+SÝu4FGL J0437.4-6155¿äþ@ątÀC§´ÃÁ‹PÀ:ÄC͵*À<¿	A=@ŠŠ}òÊ@>aÝj©Â?ĕpªä?¸± Hõ½1?òÊɽMÓÈ?ý÷børÿîWZ$8Äm?ȵ˜¾'m'¿âJ¹—e⳿ä5V#"Cø¿à| 9›Ø¿ïþb¦¾EKAGNbcuPMN J0437-6157?ïhô«?7?‡‹2é÷EÂ?XÅG Ì\?Q)ø•ox?'U*ÖQ?†Þ†Æõ…ª?î€Lbwу?¦­Œ™úÌç?dÔ¤SpæC?my*k`L?¦­ï"KÙg?¦'™êm?íëÍ6ðìQ?'Ãt[Íù?…Ua'ºX?w«Ftsê?«íÔ0B¤ð?Œ¿-™¾²?îeʤ2x?Š¤¤ž={?ƒÝýì°£Ü?r‡=Þ®?¤«ÖCð¯–?†Ã:è¦Á4FGL J0438.4-1254¿èH'™šñ3ÀA£.3ðÀ:‡;ibš)À<^÷ÇLZL@»Ç<êìó@.O[‡æ?ÃÕgûè?¦ÏÆÁã?ävÓ xñX@p¾µ²ÔÔ?Éص¹4êm¿ä¨¿¨!¿èqÐý³õe¿Üv<eç¿ìÊkÞöE¿ïÿûÎBÓAGNfsrq3FGL J0438.3-1258PKS 0436-129?ïÈüþêô?qêÀ Õ/û?GWñÃQ³?:Ž#á¬L½?x–'Å PJ?qR²y¸?ï–Ò (a¬?‡&5‹Q;w?5<Óþ+E=?IcšÎK@t?‰¡qUö:ð?†yš¶$ïä?ï-ӝ)àM?dåæ^€?l'½ž1?cü˜I]3?–³T·Ây?]ƒQ˜'?ýoò?p†*`•ˆ?Wní­@?D$:,l?‹¤£C{?o'9ì/ã;4FGL J0438.7-3441¿â€úŸÕ8ÀD¦^5?|îÀ;"xt…äÀ<ãJ?¿2°@!(dC '?ûë÷j/HÃ?̈éH-–;?ºPÓZ?ð¦<åd@›‹9¬³¿ïù_‰X?ïúµ´)h?Ù®åRп½ÕçRµ­¿ïÿÐÐgŒ?ïÿ	àÔk¨AGNbcuSUMSS J043612-342230?ïì½qGŽ0?\­ ¿'sÇ?4¬¾
E­?4ˆú[rs?`¿Ù °‡V?Z"YÝÑ~r?ï{>Š\­?s:_à‡?CHM\×4}?T}ÝMï?ûø›a¤?Ž$VÆ3Øð?í¯ûwù(9?"4ó>æyX?Œ™@5G·G?'ÚיË|?­ÙøsŽ¥?[¨ïýš?ïCëÿÃ?'s–+¿!_?`ԄÜß0?[ðÃó·1?•r…w£
?œžNÞ4FGL J0438.9-4521?ì.â'&òÀDâ$ p¹À9N¾7ޓŸÀ<Nªaâs@¨ªÙ‡ñ@c¤G?¬™šròç?¯­Hß(*R?ÿ —Œ™@/&3E|·?ïþŽäÒ}¿ãþdßӏµ¿å}U¡E¿ç0§g¸uþ¿ç­ý~ÆY–¿Ù³œÅH'AGNbll3FGL J0438.8-4519PKS 0437-454?﷛šJ
?x`VLkØÕ?=à/ló_¢?7ì*Í8?*âæ?w¤ªJ'	#?ï3‡ITÉÔ?žpípÍ$?bw¯»ëO?}áÖ´Ü(?—@3ßoGè?™±ãlêú€?ï!@LÉ<^?_$ÔåP?jœðdºFL?a¬AO:?˜"XZA+y?|òdü%?ïf¯*.¹?{™kªSñE?'!E1(?rA…¥šª?"2µó:`Ì?p"ñ/Pué4FGL J0439.2+2151?وæ0ԑÆÀ0KL<µÀ:V3sÊÒøÀ;íK¿3@çښ?ܺ@¬Ì¤ˆàå?ÑÈ3'˜?à¥e¶™…@ql¤nò@X¶ÄLˋ?ïþ8µS3"¿ã¹]¯2³¿á6,!qé¿éò3¿ïúÝ¡†M¿ïÿR@>´qAGNbcuIERS B0435+217?¼ïåo?ŸR§™ÚëT?‹Shc@»S?ŽÏ¦nœ?Ÿ!"0bô~?˜ž²[,â?é¸pŠ¡ƒ`?¿[eH$€Ô?µzÞÍÓI?³~ÊVàâ×?¼ÁœÝؼ?³†î²?å®J2Wó?°"K'ÿ_?»¬8y'â[? m¹çêZ?Ëpºúá/?ªCñ]›§?݂Ìisþþ?«¬ó«xYâ?ÁÛºdóKV?¥4¡õÁ¤]?ُVd[V?®BPIxp4FGL J0439.4-3202?éH@AtОÀD_鞔«À:}WƒÀ<†"¢¹ÓÌ@ßeSÁÉ?þò?¸|³°?¼ÂSw rç?6¨ÈO~?Æh®ª¢ÖY@±÷ò"ò¿å@XëS '¿ÖByaÀºE¿ãÜ'"€{¿Ý k…˱¿ÎÌû›Â=ӿ䔦 h?ÚAGNbcu3FGL J0439.6-31591RXS J043931.4-320045?ï¢IÇ\?€P÷7et?IŠô;´¶?FyôVL3T?…ÜŽ¥?å?~»Ê€֜?ï±gQY
?'^•¹…*?(X ¬æpä??̃üo?Ç?ƒDË;¶"É?'-f¨¬Þì?îG´^×E?!·/þ'¦?qBx¬("u?^©ž1>Nÿ?©\p‡g?‹…GóÊ'?ï:ÉÜ%E?q4úèà?E
gYiì?8v…xtJ?Šàw`é?pÿ{7¼ä4FGL J0439.8-1859¿ï'Ø
Xê8ÀB¢\þޗÐÀ:
lâ˜À<L›ó-u@؉À]¨¨?ü*î «†?»"(k"Œ?¾Íç©òØ$@}¢™ó\@?'˜rÓ?ìÓ}c.¿¨Ç(H¦¿àÿV"tn¿Óeî[è´	¿ãó·‡Á*¿ßqoC"ºAGNbll3FGL J0439.9-18591SXPS J043949.5-190102?ï<èh‹ˆ?¤´Þ';B?|©¼b?£ÝêË
6?'b®•ˆ?ƒÙÂY¯,?î'é?ê§?Ÿ{:Vð,?k~¿–›9?tÂ[zÙ¤­?¥€öÎ?œæP.Žló?í½É¦lF?•4b'k•Q?~©Ñ3ÏS]?mÃi'˜w?°'¼¨›?"n¡M
/?ìáz÷?–ŽàŒ*?‹º¾Ÿ6§?x§¹]a?»¤ÒD€yÝ?•ž£K4FGL J0440.2-2458¿Úr€&Å«ÀC‡+À:ªá»qZ¶À<q¯x(/Ê@!²§'h˜?÷<Æúû´A?Æ-—<òú‰?ÆêÚÿÀj@_l&™Ç½@ßDd¢¿ïý;)¡¹ú?ïý¯žÐ?݃¾š?¿ö+ëÁ.´¿àÏìÝ
Œ°¿Ê¢Âiq‰AGNbll3FGL J0440.3-2500RBS 0570?ï>g"˜s
?–ÎVÆdÐ?`bI'fÙ¾?Yï"Í×[È?–&ÒzÄÃ?•øá¿À?ïK18Ök?šs·@é?V³øßä?t(ñÊègI?•8ݵĜ?–âhj¤à~?íh]҅°?šf{ëã?{:—TåÏ?pË<Oƒ9?³	jŒy?˜È•Û[Ñ?íf>ÈE‰E?žáà÷Él?w¦…)(?nÜÍN7?³S¡kAõ?žÑë*'§ô4FGL J0440.3-4333¿ï/"àCøÀDÆÙßÚƋÀ9¤*ߧšäÀ;åíùm@¦'€x`d@³õ€J=;?¹»æàõ"×?Úù\ã/å¡@C!°9ï@Â=Л
¿åEÄe>Š¿ÖNØ²´¿è™'6É?¿íM%'pˆ(¿ïÿ‰b"ʨ¿ç€VÂYQAGNfsrqPKS 0438-43?ìå[ ÷±>?´/Y.yé?¶˜¦K!6?°Õó"8›Å?†rº¦ü?¦.6¥?ïiºÍ
]E?"9±Þ%H'?Z›|Ê"§?rÉhO*"?'î'þ?'^¤JIFm?âƹMè|Ö?³ü=
U±ê?ÓRT­dÿ;?±^¼a1›?¼€âÛ(g?¦k0heÇ?ï]wM×4?ƒcûëL©÷?bêyyn"?X0ïÏÛË?'óÇ9•ë·?'L¬¼•9/4FGL J0440.4+1440?àÞv,y}À4~=jΫÀ9ߨ‡s&À;³\ÜJ@;2ú(P@ÿV"tn?ÈÖMªñ?Æø´FÄ	°@;{Q^—?ýig…d?ï^"ð•(ò¿ä´ÔÞi,i¿Þù‰ƒÌÓ®¿å†D
K¿êGq®™¿ïþaAGNbcu3FGL J0440.3+1444TXS 0437+145?åb}¡ÈQ¸?¿™B馲f?ªMçгè?£õ{#Ñ?ÑñGØõF?½ª¡ß*–¼?êâA€Ýã?¹f=Ô´Aô?«r,Eõ?¬Ïœt:ÉN?»b:év\?²O‹-ñc[?äȏf½?²ƒûT?²8Òþç¡9?™cÈX?ÓP:"J7?°
¹?Û®&ù´9U?§-"EžbË?µI_D/[¨?˜@k£$Î?Þÿ5?ïÁ?§âü ÛË4FGL J0440.8+2749¿ï7ì.֛òÀ(n~¥øL­À9x
†Ñ?ùÀ;éò‰õ·¨@ $~Pg÷`?ÿU0cu^?¸ÞÎWˆ?¸ç÷±¡@Ⱥáè½Ä@6ù8¶¿æ£ùdo¿àTl~Xu¿ã…‡"ݘ¿ÚÀWVP¿Ù²¾c}}Ú¿ëÃßóðþAGNbll3FGL J0440.8+2751B2 0437+27B?î‹øzºÐ?œwõ	Îö?s.¯¶ÃÓa?pG¶kŸ[?¤Ú¢h»Ø?š‹ÚZÃK?í0ñÕÝAà?¹^'Ta%Y?ŽöÀ?ù\ñ?¤F¶AØ-¸?²™™IÅc?¶AŸÍä°L?êäãÿù1Ð?¤´(®†]?–.ï¬C'?"ÌëøÂu?Á¦'
'Æ¢?¢\l¼?ç?宎¯¯ÚI?­³xqáÅ/?¢¯|'"ÞÍ?ŽüD_Ðwª?ÒLóm¯"?¬Khuðª4FGL J0441.3-2617?îÚôœŽZeÀCÅ'U°6À;ù>U¦$ÂÀ<ý/iz@"_Ë1í
	?ø…ÇŠm¬¬?×ýÍáéO?Ân³|n»u?êG-ñªÒ§@|±¬_ð?ïÅF%~>Ê¿ïç7a–
?èìcÔ¿àùþ"ï6¿˜¨[ÜÓ2Ë¿Ò`UÀ¦Î¶AGNbcu1RXS J044120.5-261659?ïp5rkÆf?‹¸è3R?B1{yP">??Íy¥|?'gÅÖ¼²*?‹,Ú(:X‹?ï,ÇQ[•:?›AêBÁ˜?VÕEaHk?o'"?˜ùÁ~xÒ?˜×T¤'‹¯?í€M J?—ÌÍ%r–â?m\	*¬È?dÄt…␮?³%M­"?—]8k ×?îL±4z¨?™~äõ³·?3[®[=5û?4®Oì²bþ?«͐Û#?™EúâV–4FGL J0441.5+1505?åkj°‰0|À4	ü›ÇqÀ:RžŸ'×ÞÀ;ð³£¼@!ÔE¼ø™@<êòQÁ"?Á™#RŸÊ?vX\ÇÝù?¸]†Ð&?ýòº‡¥Ñ5?î]'"ƒ¹¿ÚF\»lӿ七Ÿ\Q:¿ã—d53¾s¿×ü}"€U%¿àìm|]]AGNbll1RXS J044127.8+150455?í7šzR˜?¯íZm?t"@@UqÇ?l¡ÖRéª?¶Tÿ((?®
p)G=?¼Àï·?¢:|6@ù?kÑQÏúdB?{1G©N?£YŸñ^C? ýàÍw??êHk£•æã?¨Ô½³NR»?°ì2?|¨;¤?ÄÎ-ïRFð?¦öζ!2¦?ä	,F?­`ÏÙbC2?'‡ŽâUª?ƒt—ï	Ê?ÕßÍt݂?®É;céû¤4FGL J0442.6-0017¿èu#:;À<v\=îxÀ7æ#ú±À;¦$p!Ñ@4{;4´h@ßýç!é?•@†Êñ?±¯=oÍ@ÃÀ;ÄÒ-@¢…pµȿÓc?ò©€¿ãYø™Ú¿æ\Ëè¡>ª¿æ••"z›¨¿ê¡Ù¿#–Þ¿ïþš¥2TAGNfsrq3FGL J0442.6-0017PKS 0440-00?ï®Ç)Ȑ?xÏðÖ+ß?\püI¦	à?Säs3%?€À0–?wŠô|B?ï¶9Ç;^ò?†¿™Û
F?<|'¾…$&?R1rÐ?ª48?†	ôÊ:R?ï2^c»—?…F¢"I¸b?wK]Sئ?qܵCc*?"Ð+3–à?'u⤝–?ï÷o'Í	ò?A_Má³}?#œÈÔВ?bâ'	áþ?MZñ™£(?@+{"«µ4FGL J0442.7+6142¿éë¢i»Ÿ@$^°ËæÀ:2"ѼsÀ<:ÏߦÄ%@ ö}¼ÄA?ÿÀ©"£˜÷?¸F x[Š¿u-¤Òîá?¾¢8FîQ?ú"êpvµ"?âÈ9À.¿®¾NÀézê¿çf>ù:!¿ØïõÆÁ¿Ý"F¡$'}¿Ö¨À(#¶AGNbllGB6 J0442+6140?æmžÐ<l?ź&«UÚ?~ѹKTôQ?q‡GÃ
?Òª{Ý23W?ÄùŽ¿ë?ßÛ¿ô"?È
ÃH9%?SÂڜOI?—ßrMúÝ?ß*S)6‰|?DZ—bÜ¢-?ê0N•gãÐ?¦Cf½'?Ò0ï†wi?wºÂ§÷4?ÅA¢›h	I?¤ÿ"Ð
Ö?æáH·Ó"?§Á³'¨S?«x`ñ;Òæ?•ßð5†^?͝Š Ñ¾¼?©®úf4FGL J0443.3-6652¿ÆŒ›l¶WÀBš-û¹À:@èþ[»À<t>ÿðÈ@û>¥,J@'Œ¢:R?½PÓs?¼f7íW1?ü°qgKh´@
ëc€­åV?ïúŸmîðä¿æ¸à0×¹¿äƒ`½Z¿æ=ø=éŁ¿èè®	"&¹¿ïÿÿ&¦³AGNbcuPMN J0443-6651?ïϹ?t?mb4;š˜?GñõUÉ_G?D÷֏Ñ÷¥?u%25Œ"?jíÚI`*?ï†Nx§Ñ?ŽÝс¨l?Aâp´d‡õ?`0+å"?NW֏Ã'?Œ³»‹SüÁ?ï(>`Ô>´?€VFƒ;…˜?m€Ú3­s?\V
™:¤€?—H"*1³³?}G;`
.1?ïhC	]r3?u·&P‹$?oä
		‹L?V^(ÖÄç?ö:faL?tT¹(N‡4FGL J0443.4-4152?ÙÉjF¼¬ÀD{BB…À:ôG1ùAÀ<±æõlÿ@ €ö|²Ã?û…‹Z;µ¹?Ènþ"n\?¿"xuœ9?öÑPüDŠ@'°f·š?â=Œ²­è?Üæ´yý¿â©ö©L¿ÀÉljÁà5¿ã»aÕÝ퇿ߪÛá<ÆZAGNbll1RXS J044328.4-415151?ï@%½Á˜Å?‰&–5¸
?XËsכ?ORûaK$?–yېm¹?ˆ˜Â¼"Ü—?ïMìYê‰?Ê­h	Úø?N-ª Qk?YÁîw ?•Q/q¬v?ÑǼhí?î¥yT=¤?ÐRèÈ?r-þ-?\"_ºû°Ý?¬`*Xeö?Œ%¹C~?î@ˆdžrL?ˆ>2¿Cª¤?}˜²à;CV?i'MkÍ?¨DcZrÉ?†6Ñ5
°j4FGL J0444.5+0719¿Ðù·Ç,#õÀ7ô§Å¬GÀ:W«(7V®À<"O¶
é@¼R˜©.¸@yŸâÚU?ÂVy^e»ò¿›àûF̆ñ?×>;"»f@	úõÕÓ¿¿þëWýB¿çÒ(¡‰Òý¿ëeHŸ5Û¿ÕñŠ;­«¿ïÿñAÌ(7?ïý ¿¨¡õAGNbcuPMN J0444+0717?ïËÇPÙÈi?«ž´~ß?p[!zMê?«tNOý5?c'l1úÐ?bÒNˆëR7?ï›b€?‰r×°ìÞ?BÐÈÑùd?ZDƒo±/?ˆÿZï@'?ˆ´ƒvÿ‰?îÌÙVö"_?ŒåO³²¾£?pù2{ï¿?f0ñ8!r?¡DA$ü?ŠsZ¡rp?ïªpÀÔ?tRQõ¨?MR¤‹¢Æ$?B1
¯ˆ?0?ƒŽ¥°^´?sméñöz4FGL J0444.6+3425¿¸ÆO±ÎWÀmtO]5eÀ9Ÿ¤¦=À;¸Ï-Ðã@à²;Qæ@™ÐcZBl?¼5ŽäÒ?­ê4"ö?óÙ&­ó"@M£ÔfÊ¿»j^˜'±Ä¿Ò£®Zñ¾¿å^ü_ag¿Ü^î7€ŸÎ¿è,	æ~O¿ä»ÁŒ§ÄAGNbcu3FGL J0444.5+3425B2 0441+34?ì;bÞV"©?¯ιÖ7?oÓ/õޓ?hàI/F?½&O"Ÿ;Å?®Mß[óD?é$Õ™M?¿Šxé™'?Q9–jÒ²?a´Ñ5~˜?ËJ8ÆÙa)?¿yó\ìç;?ìS,É? ›Ï¬ù›?…‡³oá?tN¤eS?ºµ¼¯é˜?ŸŠá¦ÒÉ?ëêæë̖{?'Mµ…Ô;?ŠE`ž=Ð6?mj4-Ðüm?½`Ó'%?'"bÑ¿å4FGL J0445.1-6012?ï"©LPLÀClX£/D'À:£ó}:¾BÀ<®þs8@ìVò8Â?ÿFŽ¾?Âæ¹G‰×Z?¸`ÏΉæH?õ>.‰€Fâ@	lY夊?ï›h zÉË¿êÑùÝQ)h¿ÙJM@¥Œ—¿ß£ü>Ty¿àŠÕ±wÝ¿çÕøÅyAGNfsrq3FGL J0444.6-6012PMN J0444-6014?ïïxS‹7E?X¸~RÂ?%À›×´'?§=¦p$?^m@Ö€™?W¥[ê1ÆÎ?ï›1¦J{W?…âÈ¢ˆ.?/>"äû•?@>Ùó[³²?ˆ¶áÍ;2?…r­q°Û5?ïZ…=$€?ƒQS¯—]§?cC{ÒÜ?]5›š²?œ,?Þ-@?'£µR.ê˜?ï'#™?m'ußw¡?Q7'%"4?<ñÁ|–â$?‰V4ÔË»?låõRÔÕñ4FGL J0447.2-2539?ê4z8³ÙÀBÖ5"_õÀ:ØøúRAÀ<¨!S6Þ¹@Øée´»@>ª¢ÖY>?Àh‰@ÛèI¿©ÒçÃô*?êÇ5žd?õ'¡Æ
ëÑ¿àôÈý¿Î(•µßJ~¿æהܛvé¿Þ)–|XÁ¿ÞµñäíU¿ÔÖ[[	fAGNbcu3FGL J0447.1-25402MASS J04472149-2539302?ï\ŠŠ»–? |s·'?iÁRíۅ>?ì‰=­Lã?'6"JÑÏ?‰›!S©¥s?îßCåä†?™?Ÿ¢,û?\d7Þ«&K?d›ŸYe˜?¡(¬â¬^`?˜
sâÚù­?íìý¿u‰%?ì9&r#?yºuVg>?hðÜ÷^?­øàÙü Í?
¤BDlÁ?í¾6
Y!?'H¨Káð?"Ö‡/'ß·?tù·&¡Ÿí?®æýC`uô?'³Œ×k4'4FGL J0447.4-2747¿Üˆ¥	S)·ÀCbäѦÀ<SxM¸À="—jpÐ@ßÀ‹@ÓM"îê?Ø«¿Á¡u†?ïô%Á°Žÿ@Ð=0ã@
òi™ÌšM?î}I׺f™¿ítw Gô
?Û
Ú¤{Ë¿ëžñݨg=¿ïíØë¿[¿ï PØ_¨AGNbcuMRC 0445-278?íHRG_?ÍçxŠ?'R4òMpf?¡ˆÚÜät?²Ù013ðï?À¸CøM'8?襪€ÜS¹?Æ\åõ©ó?´Ãq™ˆµ?¾Þ"*ºÞ?Ý/ʧÁ?¼rÊeè¸j?èH߁Æ6í?­ŽŽ'TN?µ×oèï?Ÿ½†Ø8^?ÄUA\¯Ñ?¨cS?="Ó?éýõðý×Û?´[Á«c'?¾·¨pÄ©@?°ã®ýŒ_ñ?±X¨L—ë?¨¶A'›%4FGL J0448.6-1632?ÄÅu—© îÀA8:}ªOÊÀ9mÆÚD""À<OËn@/=ƒC@ò?ýq½¥è\?±]!™,â?­r¡L%@!
 ë2@aTåµ{ø?ïØRÂD³Ž¿Ê¥ªžú'¿à+ÄÿÎ׿¿Û6QØ7¿Új©Ø«þ¿à­#^ÔÌ¡AGNbll3FGL J0448.6-1632RBS 0589?ïfà'HK?¾<àÂi1?P°ôO³¯?EsîR÷‹?'1t¹'û'?ôï"V	?ïiAªÕié?'dÉ^ï?H».ŽSx?_×Þ¤Žµ?'ñ0â`>?ŽÊÆÈî?hó#…?ŽG² ã?q† DT£?b»aßÝËH?¤C¥pÅ=+?Œ|Ôä%K?î:/çƒE ?‡¦ÛÄ8™À?zܼÏâ-?cùÀdÀ"b?©åð1©–?†>˜ˆ˜%4FGL J0449.1+1121?ÞâÝN"ûÀ4¼«Oœ À8-e•†¢À;'·îvï@¶Ä¼2ã@ewS?¡âއ	t?ÁÇ­¾"¥¿@©qÁ
{ê@À×õŸÔǿјº¡|¿ámm "Êþ¿çga8)<¿ç¿]¾L+}¿ì§%pÔ)¿ðAGNfsrq3FGL J0449.0+1121PKS 0446+11?ï²Ã,ï—?…ð%¸ø?kh¦1êÉ?luºH²R?xê!ВÏ4?€"èLZՖ?ïFûÀ¸Æ¾?˜Ófõ)ÈÄ?qþ,£l?Š¬L"	lÍ?' üÀ&$Œ?"¸õzÃu?î¹¥K£S?"¶Y\B˜?"r2OŒÎÚ?̸9Ç?•Y$<FÑ?"ù¯¢ý.?ï ù&.=?'¼1 ãÎh?ƒVý5Ä¿2?s[âpS†?'5\¡—Øç?|Jî	Y4FGL J0449.2+6329?—ýÈôú@'Ía€M˜9À9']Šõ'À;¬Ê‹¨?@ԂTƒí@íhžO?ªÐNâf<?·AªoT̋@Cf½Ë¨@C4ò% ÷¿Ú%a#""¿Ó**@Ejm¿á³hãh­¿ä¡÷ÁÃu¿åÎÀWs"\¿æž£Ä•ÇAGNfsrqS4 0444+63?ïÁÅ«?ê«?r|PÛC.?Göòº‰ù?B>-ߏà?|LÊ:??q×"eĀ?ᅴ»+"4?ƒÔäJ+S?B™&È)@?[')nÔ¹j?}Þý©`í?'ÐÂïã1A?î	‰»zí?"¬ÙßÔ`?‡<±Ä4í)?};ä–K‰·?©˜7×Quþ?'Äþâˆ/Ë?ï¾ÑTü]M?ic-ƍ?AX·±ýU?2àÔr¸Ñb?~têjÛ9?i•gˆ4FGL J0449.4-4350¿êœáçTýÀCõâŽÕñÀ6ä˒:*À:À>ð֗Q@vµú£IÇ?ûþÛ<Òf?'¯­|r?¯­DË@Ö"Ì«?@Lêt'š?ʜ­	ãل¿Ó¥"EO@¿ÜA¤ÕÍ¿×ÅP׈èq¿á*½]Äu¿ÚôZƒGsAGNbll3FGL J0449.4-4350PKS 0447-439?ï˜\®°º?n֚ò.+?L®â½¬Ÿ?IÉ|:Z}?ˆæ(,ÖS?€ö•[-U:?ïLç:ZËÞ?–†üs
˜Æ?X²èÏFˆý?oí}j"šÝ?"×ê'²Ì?•Öa¤ð-?ìþC 
Q?¨uÂí^G?'êº?ç?ŒJy,†Ö?ºµ_W;Žý?§]8G²¥?îD\ù±ÎX?š!{…¥ý?_Ëý9t·?RÈÛt"Z1?ª¾"ùNÖ?™ò)ùÓ¨4FGL J0449.6-8100?½ôç0–À?cà·õ¥À;À´%tÀ<ží$[)@ êÿ	àÔl@¦@×`¥?Ãþa"Õ<]¿½n¤ÁÁ?ù›ÞM'Ðÿ@*¸¡Çx?ïÿ¡ÁnT¿ïˆ_µr=4?Òed®¿ïõYÀÌä¿îO²
¤Ÿ?ïüV'TàAGNfsrqPKS 0454-81?«¤?¢ÔGÝYÊC?rkÉñVÛÓ?‡F‹â3µ?™VIÔy? ä~—"#À?íþü̪Sñ?±ÇC[Õâ?€ï²wBW?–\ò£ÈÔ³?¬
wH¼ðZ?®hî-™??ìZ'g&<?Ÿ6C¨ª?"Ý
_·û?‰~^.¼@'?º£t*.à#?œ@ŸêZ?çYC…ƒ?¼O³"…'?‡Ž»Þ_åM? ¯}»?БñõÐ?¼7™
4FGL J0449.6+3027¿ßîýy=ÀÀ"GýœÀ:4žÝ¦8äÀ;¸sQ0t<@	=-.@¬œ[ùŒ?Í/5wÜ?É9(Ö
b?þË|j´ª@å¨îÌ&	?ïßG"Ô@_¿å%èâ­â¿ë@óæ¿âW'X\¸h¿ïéÄ¿¸T¿æ$AÓ´óAGNbcuMG2 J044950+3026?á½Y¯+?Ɣ<çå\¬?¤?J––é?£ÅO¥Ø?ÙþùÎôˆ?Ũ‹½¨¾?àÃoßþˆD?˄E˜[)â?'Jɧàp? \{"_ƒD?ÝTs¥"èx?Ë+ÒPIh‰?ãƒë:û?®9'Æ£çµ?±´,D]çd?˜6Ô$Ù»?ԋìr?ª¤Åm,€?ç×""[?¨YM_4? ü»¯äžt?…çs!Ué?ÏYt§|†ö?¨Ah°SM84FGL J0450.3-4419¿ÓüL»´:tÀCáþ!ÙnœÀ9z:э%îÀ;¶íª'æ!@\‡à‰˜@I©|e¬,?¶9Ô1;·?¸}BöÊ¢%?ûÕv¿yþ@æ}"¨¿×XÝ|Gy;¿äÓI¨Pí¿êŸ¾vÈ´9¿é–ß?–¿ìs§A¢â™¿îW…BI¦'AGNbcuPMN J0450-4418?ïÚØĺñ?oaädëc(?OÁF‹Ìô?P9­Ô]õ?m7œ˜€›&?k¾W6TFÈ?ïq"8¬Ü?‡ä-:ž?<P"¯þZþ?O˜7ê?‡ÁTÖV?‡î§>‹Ô?îÖ	¶?‹?ҝ<Ö?x£‡•Á?q|£%ÂÿÄ?Ÿ}(¤º?‡¦tÆMj?ï†F2ÒÒ?t†¥?‰¦?[·wçó¦®?LKY²‡.~?Š÷öLÖï?sq¯Áô½æ4FGL J0450.4+7230?ì.qK-7@1x¢Ûa»À;µ'm,À<¦µ™ª@ê«5ÎC@Å+M‹¤?ÆölXmÕF?­‹RY?ãIþ†ƒ<`@¿̀ø?ï¢S².»Õ?ïä>ÙY£
¿ãÕµ¿'¿å&ÜÛ±¿í¬=Æþ?ԁHŸ¬RAGNbcu3FGL J0451.6+7231NVSS J045109+723014?îę¨}#X?›Ãó¨qcK?|x5ü—c£?v7IµÁP? '^¸šÞ
?™°r`1Ÿ?ïxK"Ûì?%gdé=¡?WÂÆÐuù?fòÔ] +?ŽôàÆv€?•<¿6x ?íz®Qè²I?˜öû׿±q?Žmz•¯°?'·zeæâz?°\Þg·À?•Ž""/Â?ïMÖsªŽ?~p£áҞ?~ä‡+«ÈM?qK°Ƭ?†˜%?w;%Ý;V¬4FGL J0450.7-4938?Ô2z)'tÀCÉúëÄÙÀ;Pûð¦Æ©À<ßþŽæ¸0@¬áUoô@>µÛ¿ê?ųZµÙ[¿–©@€£©h?ÐëÙ!ÄËÌ@Y¶o"5Ò?ï|š…Qãø¿ç8~–ÞÔ6¿àžvþdŽ¿äZ^»w9ó¿éÀ:SÜ?¢{•w öAGNbcuAT20G J045102-493626?îáŒA?º?"ÊÈ·	ÞV?q#CÄrgÐ?eiØÄkž?Ÿ…¦çŽ¾?'Œ2o´>á?ï6!å¦z?'ÛU)¸}C?Mjøë6?[G[4m?˜S¨Ø=?''vúU?í×"þÚ?'&%Ó;}$?'þ}áþ$¯?vj€Œ$Q?­Î—Fp‰?ŽgBt£Ò?ïA	ö?yý s±Ða?eñvF…6Î?T`iìÁ?•!ð˜n?yƒP{«èf4FGL J0451.8-4651?ÄÎå>;W£ÀCÀe¾ ºÀ9ßõ}ÅþÀ<A©n*@ü3öQ«n@ÿ#¶?¼¸ì"x?¹ªiJœ[k?ú|±|nX@¥CžNl¿æ‡¸Æ…Šï¿ã!'fw-^¿ç(èÁõÙ6¿ÝÉ%8HÇ¿ïþ˜÷³*d¿ïù|´†…AGNfsrqPKS 0450-469?ïø`Ìçdh?H+¿Œ"au?&öË8ÚÈ?!W—Yû?H¿"7­G?Eøºµˆµw?ïË5§‹E?þ¢<•ß_?*ÔËb‹Xñ?P¶³Û€?yŽ†&g?)5þ¬Ô?ï4Økz$?èç)gšð?tü‡y‰ž&?skû›Åˆã?"/#.T?{N¾@"D?ïèðòDLq?U6ÿÿQ"?5…šäDQ?-EoÇÚ?d^Zg÷3?T<衘;4FGL J0451.8+5721?î$Y §¢=@ £úLaØbÀ:ã9º5ñTÀ<{‡(}Î@!³§ú/†€?øR7y…?Ó4ÖÁ˜;K?ØCP·¨xZ@óݗö+k@¡vÈ3_ÿ¿ÐO¯j¼6}¿ïÿèþ†®/?ïý›6QË¥¿Ôný?¿Ò÷si"(¿ë°Ú=x±mAGNbcu3FGL J0451.7+5722NVSS J045148+572139?æ¼úºÁ?Åa‹±Âùp?tKƦò?p{s՗#c?Ò7ÖÛr›ã?ÅEÎ#½?â⭟™(»?˝)…˜¾?}Dð^ük?Œ÷=?ÙŐÿS6˜?Ë2áo4U/?èÕð_e*P?«xhyé:?•ØùôS¥?ƒMŒf¿y7?ÉíCàâ?ª-šâK9?ìO¥Æ/"è?£ LÈ~T	?k0tEÇ?eCñw ï?¼©QÍÛF?¢ýëP›`!4FGL J0452.0+2100¿ê<Z']À,ø§ayWÀ;YzŒŽ\À<…ñÓ'é@"³Öe|Üu?ùQÉ÷/væ?Ï+=…òrÏ?¿!%¿'6|?òkÓyq@sœ§Àù°¿îÂÉ.4¿î²;QæM?ïÿXÛch…?ÝÇ×DŸí¿ã¥u«?q7k¸FFAGNbcu1RXS J045214.8+210307?ï¤ÞŠìÆ ?‡ÑY¡?0¦jÝàŠ?*µ`?êä?†C(Áwi*?‡šE½Õ0˜?îsó«ðÿ?·€]%"×?JúÿµØ*_?m7ƒP¬ö?¨TÙO™g?·^òõ>Ps?íÍ2À¯?'ÜfÙT"?k³¬2×6À?Z¶;`áþÌ?°¹¡iÊ?'|œDh§p?ì°Yjw"?©CãÛ´O?\x5<BÊi?[¿ßëÛ9Š?ºS×R\ ?©:<b~‰4FGL J0453.1-2806¿î-¼§CXùÀB"Â	$lÀ8'Îï¼»ÞÀ<©@։å@A|wð@P­Í-DÝ?£¡?Ö.ËE?¸ªÀ³cð@¼Ý!®¦q@ùÃOöb¿ÖE»ámÛ¿äêB‹@¿èô¾þØㆿê"úÞ­õÇ¿ëù÷2ú(¿ïÿÓÀíAGNfsrq3FGL J0453.2-2808PKS 0451-28?ïäÔþ¨§¦?a¶1@ZŸ¨?R

úv#<?Lh,k\c-?b$zZGã?\Ꭷäï?ï†3¹—)?"Wtá'ü?MPvût¤Õ?l;3隒Õ?Œž
*€ëƒ?'YË!Í?îð1â-¼©?Šñ'Ó;ö?'p+#–?}5ÕÂoÈ?˜Á®(}iû?†ö²#ì¿?ïðtö²ð?O ± {?Cs¢2A1Ì?9õ¸‡L¿â?U\A€ÿ]??H3ù¸ÑÐ4FGL J0453.1+6322¿Õڂö9á@(V|ᛑÀ:S±E‡ÊÀ<+¯BxJ"@ ¦ˆgB.@zlãX)?ÁJº"üq?›-¹ÌƒÁ?Ýú$Á‡@émÇXÅ?í£J¨š¾¿çðÇþ±Ì@¿èú)(î6¿ÑËaè¨K¿ä!æ­j1¿à@"°%ÍAGNbll3FGL J0453.2+6321NVSS J045312+632117?íá긼Hä?´ÙóÛVÈ?_¯'X1Æ?TúñÛGÊ?°qî X?´ÐbW¶ô%?í(áHÏ%{?¹4½¸®±ú?a¡?çK:^?|Ÿo¯7þR?¶+ëºLzL?¸ï"¾zQj?í£²ú£ú?™¼ðÅ1?wZ›¿N?fè^¥!?±rUÎnëQ?—ÇÜZ¦¬?ìUã9Úcœ?›H·Çäg?…"Î2?q6XUñ6[?º¬ŒpI¡4?›»îäX°²4FGL J0455.7-4617?é"o'*"zÀCi˜áõ²À9
¥ÿ©þÀ;ðšrÝm.@&¢†}20@ÝÓ4ÅÚj?§!­¤¾e×?´âÎì·£Æ@	ÿG¶@yX«gÍ¿¿ì 	·¿ä±Ö;áWž¿ç¥c¯˜	¿çWìPÓ¿èŒYÙ¿çƒO
)N®AGNfsrq3FGL J0455.7-4617PKS 0454-46?ï掲ÕI?\ØÃb?/Ã?B¨F>j?;}Ò¦$?dÇLi¥i÷?ZI8±hµâ?ï¹SïýñÖ?i)i;?4ºâwŒ3?F9Ïį$)?,ìËFc?€µ‹ûùi$?ïˆ[Ãü?ƒ*jبŠ†?p$»ZJÈ·?Zþ¼ÅÛ=õ?˜^€ôÎ:?t<=oÿÞ?ïÛÖޕ_q?ZK>?ÅÈ?J™bxïž}?:L¡d…d9?m'ÈÌd§:?WÛVMlp´4FGL J0456.2+2702?ë0´Ö`õ8À$0H@áÀ9µ~q'
À; Œ‰ޚ@•tÁrüw@ïÇ£˜ ?¼xtŸ¨ì?Æ.ëzâÊ:@£É%x_@ phó´m?çÜ"N‰{¿Ü^d¤ÅFÇ¿ãc3vO¶¿æu
þÆD¿èå@6&¿ïÿ¯b® èAGNbcu3FGL J0456.3+2702MG2 J045613+2702?îY>Ó-?˜á"1?zt§H(Œ?uBSQ"š¸?£¹€g)È"?›v§˜·"?í0Y¦{ý'?·¿åïïÚ¦?^-!¾"È?ukeå0m?¶~GÁŸ?·sQ!¬ø4?í*¥õÔa?œò=Rq6?Ž,_>f±?~F\¸Øò?²åG¨"†Õ?™dÞà÷?ìç0cÁ0‰?"ø"Ž46Ð?1чҕ=?jÿ
îÍ>?¶ B°ü)?"ÔÚy ñœ4FGL J0456.3-1634¿ä"bÐäÀ@^JÀ:Ý'nâlÀ<›×5Ü@ÎFtƒ‹?ü½úºpª?Ð
]O¼V?Òrsºâ¿}@‹G&/>²@ÃU¶ÀÆÚ?チ_æðe¿Þ51e'Ìù¿Û§Î›Ya¿Ó)<ÅS¿èÙÊÁÚ«]¿áœ]=ó«‰AGNbcuNVSS J045618-163552?î'PFú?–÷•¹gŠ?€lo¢TD?xäl«à›?¢¿ß§ÉçÆ?"©ªPQÂ?íäې"N?©^ÃXŸ­Á?zÿ[éÇ*?Š^¿
ùôO?®R[y…•ç?¥ÜÞR®'ÿ?íAH­½[?— Ö綌w?'-±
i…?'Ó¶2ÂT½?±«½NºÑ?"%{²¤‰©?ë¾ +^{?—Ø^5¨*?«Ø$t´?xœÚƒvI?¾Y"2uš?–ƒ4Ƅq4FGL J0456.4-4043?ï•4•¼rëÀC:-ƒÆÉ~À;oºzº±AÀ<ËÆ+ÈÛ§@úu.«9)@ü!ƒÞFr?ÅEÅÇtô¿±Tÿ5Õ¥?élґ1ì@ý½Èäá¿å3!€nÅ¿ìé ¹³ë¿ÞžOv_Ø®¿ÚMõÏ¥¿êkŒÞl²?ËÞ3<ˆ]AGNbcuPMN J0456-4041?ïÈ;¨çß?óÍg$</?J¶Ž³5}?N¦|–lÉ?x‹¥U%`m?€Îà8ª‹?ï"_ýìÜ1?Œ¶!ƒ•Z©?7MÀÎG¼?K\CŽS*?Šm'~V·`?Œ D•ð£?îDGYéÜ?'æú×ä ?t¿pѧåÀ?v¼´Ù?¥SÍp,e"?'hÌ×d»ª?ïÆÖ,pƒ«?h92Ñ´¦¼?4ÓiÊ©ÆA?,Ðç±ÐØ`?{G³+Ž7?gé}Ǝù4FGL J0456.6-3136?á 5!ŸâßÀB‹;BÌ-kÀ9×Þuk¼çÀ<}'Õ1@êÅÝð@¥qŽ¸•?´8=´›É?µ8æÒÝ]?ùô3xÓPu@Q/¹¬²?×Îÿ¬óéq¿á­w!t™Û¿çøÃ*Œ›"¿æm¾ÌeŸ¿ê½ÁÆßM¿ïÿ°_ïÉAGNfsrq3FGL J0456.3-3131PMN J0456-3135?ï'[18ØZ?Œ¥#Èç43?fNƀ(?_Bñy!6?†'¿èÄ?‹nžB³åñ?ï£%j®?¢ÊcÁ'ñ#?i8x¹ˆ7?Œ\•ÿú'?™DŒGá£^?›Ÿ‰aÆ?YF?…ðvâ$JJ?qm¦ë7…?i/2á"`?™qbš	^?'áh©f?ïp±)QÛO?v–@â¥@e?}FïÓF?m_A¾Y'?'Vn¼lXë?jžæJdؤ4FGL J0457.0+0646¿àq0wt´;À5«Þ灃ùÀ:­¸4TÀ<ùÅS[È@/©RtA@¯U!š"?Á­‹¾åƒ}?ºF6mÐ=?ô—'ML¹í@ç~­Úï$?åïB]r¡Þ¿ÜK"]xB¿æ韀äA¿éå.X•¿éO€pÓ¨¿ïþcèݤ‹AGNfsrq3FGL J0457.0+06434C +06.21?ïª`±Ÿ©Ø?¢î—H9[?Sn!›¯°ö?r_•£
¤‡?'údŸ"?¡So3²÷:?ïÃdëʾ?¬«ë5û?/Öh6§{?BH÷ߒí?}UUÖØën?VD`¸?îÜ;NU?ŠF2=ÆÍÑ?t±Eí;þ‰?gLÕÜòØ?ŸP'$‡5¹?‡
ø~uðN?ï€$?hD%?r4E–aš/?WÇxÔ²MÛ?BЩú¬?ŒþX­?q">t
¶#4FGL J0457.0-2324¿éVXÔNîÀAs;÷'À6q%»{k±À:øu/@­!­ú¤¡@ξú|2?€a—Ó#‡?³YéA¢@*x®I#`@ ȋ÷o¬¿Æ律4ë¿ß3âÂ\†¿ä~!nÑ¿ã¥cœ‡Š£¿ç{4ßZÃñ¿é@|ÇÑ»IAGNFSRQ3FGL J0457.0-2324PKS 0454-234?ïWAÕÙ¶?ˆÔæÝ»F™?GumQ[÷ß?E"%nWðk?"RLZ¹é{?ˆ‰€=@S?ï¤Ã/hh?¤-"Úº§?ms)?‰Ð¦ƒ?šÝvO²ê?¡ÁrXA"?î'܋%D?šÙ)ùø¤?Ž§õ!€s?70».‰Õ?žiéã
—<?"ôf^ЋŽ?ï X'³M•?&N¾j?XrøP$}+?[i~òé¹?"Û|I(V?€íR4FGL J0458.0+1152?ïWF"Ó¥ôÀ2¦šíV°À:îê'ò#À<R1Xg @!ǎàV?ýÛRUÆÜ?̈́`¢W-c?™8 °d?¾žœ7ً!@-TÔî"X¿È¬Ãœã%¿ëÁ!h/"B¿ëÍÌsáy?Òó½‰bë¿á‡¦RÁ¿ÎÿùŸé"ÚAGNbcuNVSS J045804+115142?ï>·0bª?"•ú'¤¯ƒ?:[ž‹€Fx?:5€´Ë(0?—¿«y|¼£?"að·Üž1?ïZ½>韚?™ÍóNJO?Mgkv՜û?lµB÷Æ?"½Ç_ú?˜æçuRq?퐬à1r?›ž'1Zќ?pe…Â×ËG?`|¨Ã-Êà?¶Å"<Ð÷º?›${>2ô¦?ìÒ`¹ßâ?¡ñKŸ ^?lf«>m?h="€ü
?¸‰ÄØîÿÅ?¡ÐËJ'.Ù4FGL J0459.4+1921?ïÔ5ŸcÍÀ, æ)•$ÀÀ;"ù÷¨À<BŠgÍn³@!ë‹Ô´ù@!Mø±W&?ÎM/Ége?‰régÉN#?À&¯X‡@l5%Ñ¡¿µ@cÖ>;?Û7½;_QŸ¿î˜Ù`ð?ßgk^Å"¿Õ;ˈ).Í¿å@¿ã°>AGNbcu1RXS J045931.5+192242?î¾5Ìda«?¢%FIWÒ-?VØG§
°¨?i}`6?£eàüÃ?¡ôö3?ï‰(E˜ûl?¤çtŠ·z?9ó—ý¾±?`¥ t?ŒæU½6¬?¤I†»ŽÃ?ìåÓ^=?›ÿ‹5Ì®Ü?smÁ+i§?eú>Œÿ¼?·œ5PÎ|î?›N4Wú•??ïSJ$àÖî?†ì#¦Ƈ?Mï÷牃?Mê57cŸÀ?"§;¤¨Ö0?†{Ox^¢4FGL J0500.1+5447¿ïùúÙ̀@'r%·I®À:žÆ3¡îÀ<,©ã"¸¯@Ƃe n@±Âþñ´?Înø†9?À±½½:]Ÿ?í=Àgc¼@Y9Ô1<¿ïÊô Pm?ïºiúÊ¿èín˜dt?²òpËD7¿ïÿø]ˆò?ïþ÷ýÖÛAGNbcuGB6 J0459+5441?ꠊ;ØB°?À^¬`ƒ°y?…Ü­j'?‡¹'ؘD'?Ä 9þäŽ?¿\•íãÔ?ê:
¹µ?ÆÿÐ=")?}x"ù'EÌ?'7ÿ¹¡)?Æ,1O'þ?Æ4qÄ2ò?çý°ÜÍt-?§ü d
ù?ž©ýµÀ0u?‰óTOãz?Ì3üÖ)=?¦i͝€?íJnü8´–? ÙþG{3Â?Œz°÷c`?'ºŸS+cE?²*XÈnä?ŸBÀ;c÷4FGL J0500.2+5237?¿–a°
Q@fL¡™B\À9ÖI°M:EÀ<ïH!×Á@!\$˜Ö¸?þŒý"$½?³ÇÝ_þ(¡¿'¸îª_å?߅&šôb"@-Ÿ¿ÛÓCÁð?ïò¥­Û¿è]¶Šk¿Ý– 7˜s¿×^ÎA–ù+¿ËŸ¥aÎÒAGNbcu3FGL J0500.3+5237GB6 J0500+5238?éšiÏW†?¹«ßYzÅó?ƒÚ&@°d?x¤ÂóšÁ?ÊCó÷N–ä?¹ ¨»ûÚ!?æe'?¨?È2?I]Ða?t^µé;?!·gT­†?ÒäwDa×;?Ççþ˜{ÖT?è›tÀNÖp?§
®epä?"çJߪ?}jŒØrD?ËIµh°ý?¥´ä±Laç?ë åàsëc?ž7›£‡?™ûôÕÙ?‰tÀэ‡?¼yÓÇ.§?ŸmbӐáò4FGL J0500.6-4911¿ÖÑøì̃ÀBý@=ݱ!À:­Ž!–R½À<Ÿù¬ÿ§ë@ [»=XP#?ürùà0W?À5AU_ØÙ?¨äEdc+ô?ì¨OÌû@Ø×¾˜V£¿ïEFáeá?ïÒÖ0ù¿àFÀ¾Ìƒý¿Õ0ÀRŽ¿Ý"¡}=ÃZ¿ã•[$AGNbllPMN J0500-4912?ïïSË£G³?WæMʂ)•?, ôùeÝ?&±UH;»'?]ÔJCöì?V)ÇÀÍ}M?ï¹ÛÝ^±?‰H¶yú?(WŒÍôOØ?F~Nzé?'ªuG'´?ˆÜ°Yö¸?ïÔ8E¨J?€XåÐ?~?c)>f° ?P®ÿd¨¯?šQ3~ °?~ɮՇþG?ïŸÇhŠ£Y?iž@8âs?N¥:ï«ó??«ÁVÈiB?†#Ì	¨/?h|}î¹ä4FGL J0501.0+2424¿ãâÏ—àÌÀ%Š|àü.ºÀ:à{ö£ðÀ<_c>"¹†@!W¯K‡'Ü?üÄ<"¸?̒üÇf[?Îìì¥@°ý¤?÷éä4È^©¿ïÿôA…ÜM¿ïï&"è±?ïÿü9¡â=¿Égâ<u§¿âð!愯¿Öv"œ;AGNbcu1RXS J050107.1+242318?éÛŠ"Ô"?ÀeƒBq?Z;eœ¾Þ?ZÚËp·°?È_?¡t4?ÀP€.
?å0xÍH?΁>ÚÚ5?'?ç·C³«?¢±µ—Oz?Õ
ùЫR??Î]εÕ??é‰i*´Nc?ªØ¯æH5?"%Ð¶ù}?€ô§ê#Ç?Çu©›çF?¨×u7Ô_x?ãåIÂ?µ3è%ÿ?"OÞ	2?Ö,]Ðú¨?Öñù‹J?µy‡/õôÆ4FGL J0501.2-0158?íÂ"kÀ9J]ž@ÈGÀ7­†!ÐýÀ;íZQ@x…v!@$Q2øzÑ?–Ö+Ú¤Q?¶"À%@ϼ¡Ÿ@‹F¿Å¿Êɹà<¿âl•õ *­¿å©Æؗk¿åFC¡+¿êңܺî¿ïÿ½ÅGóAGNfsrq3FGL J0501.2-0157S3 0458-02?ïÏý"
Χ?j‡$V‹½?Vƒ©3Àq?TáAô7=?r`"­¨|?f‹±¹ºI?ï"=BNõÔ?•/w´©t?Vu'zÑFw?z_õK?Œ!ý<èbB?"ìS-yg?ï2T›[¤?ˆL±ƒ{á»?ƒ°Î•='h?€m'Ä%¬??º)Ã딷?€=üït,?ïñuvS&|?PjM2]"?8á=Ô?3±"a¬{?Vðï!cÀÅ?K±×½‡¼4FGL J0501.7+3048¿îŽóðÜÀ@eށ*7À:hÚà‹ÆrÀ<¼²£UÛ@!aB|§E@	ý¯Ã¨?¾!°¿Pˆ¿¤¬Ž¾Ê*±?äõé@ Ú?ý÷þyX1?¸Öf~'%?ïËKøüր¿çKlD̸«¿ái%}½ðç¿ÛÀ-Ëë%¿ÌæFÆbûMAGNbcu3FGL J0501.8+3046GB6 J0501+3048?åÔµ)ãB?Â9¦áÃ?ƒ€±×W'?v
6pT_M?Õ2QóvÂ?ÁäCÈÒ?׳AMO?Ɛ>Ñ?r›ñ!Þ-~?âã¹þé…?ä'w0=~?ƕ®‰N'?èA©†"ü?ª"6\ª¬»?'£nà
®(?uÐ!ï¡?Íz‹}ãöI?¨þ;ÈIÒ?ä_Ú:ÐË?°'èC˜'?¤iž­XÕ?˜O©çì"Ý?Ô³ÿß[Ž?±ŒÇw­4FGL J0502.4+0609?æóöªÊLÀ4Ü
Ð=š•À9ÌTæ³^À;¼Ñy÷Ü@:꘺¡|@jŸ±
Ï?¿Ô‡×$i—?•[ÂéZ]?ÒØöî‡@çzÊÒ!¿Ø¿o˜¿ä˜±<MŽ(¿é"ø!å-¿åG†§NŽ¿î"6©	y&?Þh!Q‰`AGNfsrq3FGL J0502.5+0612PKS 0459+060?﨓'B¼Î?­öö-€`Q?[:®–Ýì¡?~Í92r°?'sÅÜuT?ª#Ù]œX?ïÉTíˆ?R
%¨a?+ƒ¿_Ž/q?EXŸ.Dd?zyku¿'|?€G·ò"û?î£"ûJÅ?'"Y)C‹Z?z žèïê?n7¸Îý¾b?¢zµ¼n5Â?ADúô?ïŠOém¨?sŸB—½I‰?McfÊ´JÐ?@…›´Iö?‹•Ï7꺞?s
%ζ4FGL J0502.5+1340?Ü^qš¢IÀ0»)^ž	À:&=²èöÀ<0B½ê²@)û'êV@rÜ£Úe<?Á͒švä8?­Ê­¸µh­?뢱Èd@¶5?|푿²çgWÒú¹¿åœ|m8è¿ÝïU"qD¿ã%‡
¥Úð¿â<
½s=¿él¯áY¡²AGNbllPKS 0459+135?ïvý϶V?†Ð.Æ>*?W?¨whR¤?M'¡¡>{?X— k?…ÍÓ¸åQ?ï«É]Éj¾?'"¨ˆç†?0N5S.µ?@Mš\±Ìì?"‹6ãÜ6?'JÜ}Àî?îµ|þv¥j?Œšãêù?rù	+ @J?h¾±ªý?¢Ió!¡b?Š×H‰–?îµÒ[1+B?LB:RÎ?`áVÝ9r?Id­;hÊ?£"Äߺf?ê±j"E4FGL J0502.5+3438?ì<䗙º&Àe©>ê!À8ïíO#SÂÀ;m·‹(U@¼"ŽðsE@‡z³$…?±1é\$™?À9×|©ñ@_;©#z@(ÿZ¾'w¿ÃžvãŒ+ó¿Þgö^k›/¿ãºÔ¢Y0É¿äÅÃù¿t¿é"´À;™ß¿ïù\wÐ6AGNbcu3FGL J0502.7+3438MG2 J050234+3436?í« úÍP{?©˜1Í¿Œ7?sRv «úÝ?wG©góZ?±mпŠ¼'?¨Š¬¤È†?ìŒØߖm¸?ºXÜèf'T?TF†ÈÄ?kgRƒºÏ?»I3éNw?ºIœ_›ÖO?íaÔÍãÏ?œjn×ÍÖo?Ž<kW5ω?ƒXp™Ûµ?±)Ì&?˜šùRÅ.e?í¿YD0­?'AävŸ3¬?€©óìžbæ?f®u<ݘ±?¯ßîÁ͖i?§ÀÝP.¡4FGL J0502.9+6533?çG=:j@,¢ÿm3	BÀ;B§½HËKÀ<¿]K4²@"<}ðÿ1?ú4ÉÖxG9?Îý"û|ã€?µG@†Wó\?íà8Ÿƒ¾f?ã£éõZ=A¿ïê¤N(ÿ¿ì-ã}"S¯?ïý©®º"¿à>qTÖò¿Ô;‰"%¿©æ"'ØäAGNbll3FGL J0503.5+65381E 0458.1+6530?ï9ªBåòè?§šf^ÂÝ?;Mù":…?BÏtjn×?˜]ƒ[' ?§yÕîðÒ?è	ø>»[?Éï^O|Ç~?'OU¤›Úè?¢5úô<Âa?ÍUíjq—6?ɛ@"·á?ìòӟòƒ?›¹7Ü÷uI?zÜ»o\™?q…ÿɟe¡?¶Á²yv?šÏ;/B»%?æ·¶kÃ?¶^;¦ý?'ø¤?':jz ~?Ò¸h7?¶&#š-õ14FGL J0503.1-6045?ïø¼âÃÀBG¼Â"çÀ:Ó^†žSÀ<4¾ÓåÅÂ@^Æ1Ó@.v]Tní?ÓÁ1ùwOÃ?ÙE~ð ç@`Ũ]_@†lQ÷?ïûŸíp±¿éq'Šˆ"ž¿èîwÂYV^¿è(¶½–Îä¿æsûŸóû»¿ïÿ.ÿqå¡AGNfsrqPKS 0503-608?ïÈö"'=5?xK.i—D?p;ð¶E?qÙ
Åx?gMõá_x?hß°âcÌ?ëgÛsGÛ?À(aĵ=¬?¥.†0je?³;š*SÎ.?º0>0Ž¡?´/Q>2?ë7QŸPƒ?£¤‡ƒQ?¤×õîwp¦?'¨_éê™?»Ùx@/Q?Ÿo}Ål?è»Á†í?®‰Ç•ÛÜp?¯ÍŠd@·†?œmPÝÛã?Å™é¶e?®Bë^€ù†4FGL J0503.5-1116¿ë½Ô6xÀ=âÅ\–À:˜Ä0FéÀ<id»k{y@ žMQü?ýHò'hûl?Ď:?ìÕ?¬
rIÉw®?æSò@#Ü~@'Ä{D™ã¿Ý'NÜÜåI¿ÜK(\ëhn¿ßÁí@	ÛK¿Ñ·üƏ›ê¿â=U–4ŠK¿Ôf%ƒ-ùAGNbll1RXS J050335.6-111504?ï+Á+a?766²Ûª?I—ªß¶¨…?;w[Ì;*>?™Ð
ƒ œ?ŒÅ¡?ïQÍdï̗?™'oª´¸p?CÏ~?ö¡?W é/4?•'چms?™A^Ǽ½?íãhcc¸u?'d/³
*?txkƒ(Ï?`"‹•~?¯:lfT'?'j_eÁºŠ?í̼٣eµ?Œvtƒ ¯?f-Õ?SûêÉZ(?°é(av)É?‹ä½€£[C4FGL J0503.6+4518?g"Nô2V@ŸÁßeVÀ9¯Üöæ{ÊÀ;Üè,¤£¹@ ¹uj:[q?þ•i‰0–?¿â=ž4?»ïÒ Ì=Ü?ý2Ú}wØ@%™¼Úç¿ì¾²Ã6K?ÛS®=j™§¿ßväOö7¿Ú"¨~cÞ!¿âX>à»l'¿âì&ďçAGNbcu3FGL J0503.4+4522GB6 J0503+4517?ê{²E¡?²†Ñ¬»H?sÀ,Âü_?j§ŠòÂ?Ås6'hћ?²EcM,ÐI?æµ5ÆÛQ?ÄõÛ²‡dà?|ˆd(V:?«¯CôÞP?ӆrá¨?ÄÓ~¶ˆWŠ?éxÖo?ªn(½Ñ?"É| Yi)?ىXŒÿ?ÉLí÷áy?§åŸVðÀ?éšé
€úå?šûö†ÿ6?šM·pº?€k¥yd'Í?ÆJ¸ßFQ?›N6Õ¢sŒ4FGL J0505.3+0459?è˜óò´­À4Ü9ÿÖ•À7jD†AÎÀ;öÍ0 @ØF·õOM@'Ï] Å?•€RY#?»\•­%è@#VŽÅ*A@ÕhÀÞ­¿Ë*(][Œ¿àèû6l£—¿äüÒï%½)¿åÂψh﮿ëQþ'A·¿ïÿ±[W>«AGNfsrq3FGL J0505.3+0459PKS 0502+049?ïjH\ã?"ó만C?x-Ú¿Ú­€?xG»ãRè?‰bˆÙèº?|ÅÂU%ˆ?ïŒ,ôF¢?'ù!ÌÝ?WJrÖ=&£?qkɘ-`û?Št"´r?'/}Ù?í_¸è£R­?£âqϬE?§½:3i?ek»¸Ç?¢Gk;—¶¬?–¥‰ºœ"Z?ã¾>a?~/m‰mÔÐ?Wó±•"W?R¬Vœ`¢v?…ÝPÝÎuT?|æ{"!™4FGL J0505.6+0415?Åðu™½´À50ɧ~^«À9Ì1p»SÿÀ<KŒÆL€@ ËE05ÒË?þÇë¼|?¼¦ÂÞ¼Š?¬.Eã?ï왡&UÕ@.	™Üµx?ïÒá锄¿áݳÍêÚ¿ä…™1"οÚ{$
¦\¿Ú;¼ïŠ¿âsÂóáAGNbll3FGL J0505.5+0416MG1 J050533+0415?íÞE/¦™A?¡Ïæ›/% ?p‰Ž-'?`ñVÐD?°Ýê²S,?¡Pš¤'–I?îç~\­?›·§˜šl?hØ!KÆՐ?vÊÃkŸ%W?Ÿõ0@å#ƒ?™da3½?ëx¾'š5Q?£'l¸Ý3?0¢'ø«I?x$ͅ¤È¯?ÀIý8w ?¢-8WC+?èÍç;¿õi?¢­ü+Ë2®?"••%:X?u‡­¶WŒ?ÊU°l_Ã?¢Ã?=©fÇ4FGL J0505.6-1558¿ëg'ЛbÀ>n¾‰¬½À:"À';¯À<~iœ{Ì)@_ob¹]¯@MWoÈ?¿Ê™@Ù9?›¸œÇªÎ?ß¡'à'§b@šP¦`§`?ï'ɨU@¿áÉåX4¿ÜÉ þé7¿äæã>SLÙ¿Ô'üŸ"p¿äÂßäÆAGNbll3FGL J0505.5-1558TXS 0503-160?ïY{ÔÔÓ?ˆÏô]t?Q:âˆÅÑ?C:v(˜ü?"¼×Tُ?ˆU)e.•¹?ïiæ֗ê)?'Ú\"·ÍF?=üí ì?S¬dI£g?'O9L7?'l–:U7?î½i\ÿSì?ˆ×Qܐ§?k#ç¤ûQ?aÆ®¡¼?¢y7ñq—?‡¤Älɨâ?ï&­i†þ?~¸(¿@pZ?R–=‡JÁd?Dy6ÀÖ¦?›±ÆzZt@?~©ÅĦ_4FGL J0505.6+6405¿â$^óÅ#@+kJfUŸoÀ:Í*ÀêÀ< {ÃW@+î¼@žß(Ã?¸¤³~:ž?Ň>£(ä@`ì>'Ï@	m8?ï³ÅP˜¿Éü.dAs¿çôß:šˆ¿â[?î¿êŽ›~¡¿ézNW‹ØAGNbcuTXS 0500+640?ïLzîñ9?ŒØHwp ?yaºÁo?u¦~
š?OqÆF?‰"ËHêµÎ?寮OË./?{šáØx?B8èå,¸?X7ØJc¾?…-]~ãÁ"?ŽÂüm@ß?íé•d)Õ?•Ølþ­?'íh‰æe–?…!gþt'q?¨oõz
/é?B:dH?ï ÛU#œ´?p'&ÍTD?[´þ' ;#?K"—"Qï?"RŠæÔËÇ?nóèaR4FGL J0505.8+3322¿Õ)õžõp|ÀGlãËÀ:f÷ù¡A.À<­-@ l"
qË?þÄØý\·'?ÈÝ5:I|÷?Èϐa³'?ýÛs©EH@â²_¤¿ïÿ	*K-%?ïþY¢2ÅO¿£Gt!©·¹¿æ^ú+ª¨¶¿Ò"Üޒȿíñcºº{'AGNbcu2MASX J05054288+3321355?ÞśÀnßN?Â@[¡?Œ=¬ú+ ?"–ʧl…?à,;kßãÙ?Âw²À7f÷?àYc.ð ?Æà@iñeš?d~ãÍü@(?wÍ̍ ?ß°Or'A?ÆÏ9|6¡C?åù`¡ÇÜh?ª|'mžã?¡ÊYÙÎE?ŠA'èË^=?ÑÓóP-g?¨ï0Nj?éÎ¥Fvú?¤óN
Ï¢?ˆÝà`ãôL?zòØ*Ü8?Ç7¨×äÑ?¤»Ìa~ê4FGL J0505.8-0419¿ïÁ‰ºJárÀ9f?x»Ó€À9·iþ¡[/À<œüûhÂ@«uÄ'aÄ@Ä#°ß0?µcl6	&?›m=ù"\ò?ä\õ8ü Ð@…ìiJF?ïïNlta¿Ö"vÅTÉ¿ç9.ŠWw¿â¿üò¿ì)ÞJ΅?µmôÐ!AGNfsrq3FGL J0505.3-0422S3 0503-04?﨔µÇ¶\?~{
?MJ‰¸† ??4äD=?")ýæà`?|üj¨^&Á?ïÈR¿cE»?}®% R¦?(V2HoGg?8žÈŠÀv"?{þ?|ÔLäÖ?îaqÕ>¦?""ÜÚ¶AØ?‰ w\«8œ?"?_1XÛ?£ ÄØqGk?ŒÀs5†W?ï¶(Á&í?f2t®8?RŠöŠ4ý?Am—Æì7?€$—­>+?d¶mªX'ž4FGL J0505.8-3817¿ïVmC—ÀB/@Ý?á—À:²'f™'À<ª; †ô@øáі¶?ÿ©òâáH?ÂâÍ)¾ë8?­#Ú¥¨p¢?ë)õœÏ®ÿ@	n»·¦Ÿç?ï¸Â‰|ëä¿ä"§Ös¿ä#ÁÛØ‹¿Ðð~BP1œ¿å¨Ñ F1¿ä3Û._"AGNbll1RXS J050559.9-382059?ïçƇÁå.?^ð~"4¾m?-`n§o? ©!+[?fhÂ79g'?]èøÏC?ïˆÏ
Ç?ŽSV"6O?5£;ÊRô?JsKKF…Š?$ùïÅò?¬B_‹?ï%<a¸æ?}u'l\?a´Õ©£õµ?L=y"Ä>?™!ў"dx?|]ý5
?ïnôö?se!yhF?W«9"u›?Ccº_ãÔ'?Âíêzî?réWXü¿4FGL J0506.0+6113¿½¹ñ0ŒîC@(1\FRÀ9®ð©Jç…À<&¼ßï¿@@ ,µ?½Z@'.B2ªw?±"Ï?úT?Å^ïN­?àPž¨ø@Rïl_¿è'ýº*‰?¹SŠk©F`¿æ–!W=ª¿Ödéc±UM¿æ}º«bú¿ÁSæ.Ã7AGNbll3FGL J0505.9+6114RX J0505.9+6113?ïcØ!ÞZ£?‹B,ýZk?Rw\IÃ0Œ?Gfó¤hò?']…ÿ˜x¬?Š¦^K‰?ï}Ÿ¨·¹?"4ýWB?NÇ7áj?` ے"òæ?Ž«¢Tªœ?"›¶Õ,uÖ?î…WYFá¶?dùXú<	?sHqf	å'?fE2!¢?¥A|>Чó?ŽøÓðö^Å?î³uºf?†ãùñò?ëôîCš"?lG"Å{N? M§#ø·ã?"¨ââ|p4FGL J0506.0-0357c¿ïgёhÙÄÀ9-DŽO¹À;{È0…ÙÉÀ<â¾|§ñK@  czΨD?þñìVuX?ÖÐ^ÚÖÑ?éµ°P•CÊ@
h¾/?ÿ-å^0´¿à­Îod;ê?ï"E¥%¾Ö?Í91d|'¿ßCµA?æJ¿ãð"aùð¿ïÿvä܎AGNbcu3FGL J0506.3-0357NVSS J050605-0401520?ì6r}òH?µÛҜàܦ?ª™3˜?¥¤
änFÌ?°ÿàvâ¿?±—ïšx}?å"]'Ÿó?ÆCµ^ܬO?Åo6czIh?Áé;:놶?ÄU6Í?µ†ªþ}2?êE!ÙW?¨è'"!r?²Ö(?žqØ2cç?½P'ÂÉ&4?¡Pmé>?àŽJî8²?´¯b٘àñ?ι"÷†6?´•Ýzè]?Ï
R¼Á?²¦_å'1.4FGL J0506.7-0857¿ÁÑ$øT\pÀ;O¯§"YÀ:3+y*ŽÀ<Y^¾Ò@"¾ì‡@Ÿ.cÀ™¹?¸3°ÜJÿƒûW2'?̦WB1(@/DŒ?ïÁ6á¾vs¿âØŸUd¿ây,Áÿê1¿å3+;-C¿ÞÚhH¿â¿ÚÖ­@•qlAGNbll2FGL J0506.5-09011WGA J0506.6-0857?ï5`^p"ù?£¦†Ň?_¬ "<A9?f2S1"`?—Y*/ɼð?¡ÃòD¤e,?56:ã?…Y'q=؀?6öé.b7?C›~ë:>G?ŒœÂ›'ԕ?"Ä'§IW¨?û|Qü?‹+²Ž?s(JÖñú·?dWë*6)?¤Fí\ û?ŒÑ¥éÙ»X?ïBKh?V?u½ƒ2å ?`bÙjnª?M-ªƒÓ¶õ?•ªPçîÎ?uº»{ª4FGL J0506.9+0323¿ç9mþqpÂÀ5\ÓZ…‡"À:wO"¼
À<ZÀ2Š–Ç@ Ja·Õï¶?þÓۙï)ï?ÁÏo¹Ì?¤)JQ1öÈ?ãO]¶>–@Û̈́ؗ[¿è—¢KïÃ?ïé%=QD@¿ÛÈ*;<ìð¿âP7…¨K
¿ãJ™aj?Œ5¿28!AGNbll3FGL J0506.9+0321NVSS J050650+032401?@Ώ?|‰!TOÂ?U]é¾³A?NúÞ¹½t?…0ö'"…P?z÷#&Œ?ïgÈÂs‰š?'ocï	H?J‹'¥l-×?Y­‡"g"?'2‹œck|?e
4Ê]í?íÀx£Ì–~?"i{¼Ú}?}LÚmúa?mÞÖ£¯x??°'m:»¥ò?'Åö•Y€m?íÀðDc?oˆRêì?É  ?kI‡k{§?¯÷Õ#HeÉ?Žá…í¡W4FGL J0506.9-5435?¹å ²`×ÀBb‰üm¤HÀ9·zn['nÀ<D€bï@ }ëišù@?öb¼'«A?¸p°íOF?ÁÃÆé³ãG@ýöÀ¼R@èWº§¿ê°Öâz^¿Ó³(¶ØnÁ¿É1£:৿ÇLíCÌ¼¿ÕH[¬¿Õ<{ÜDdAGNbll3FGL J0506.9-54351ES 0505-546?îôl—´^¾? ÔD=à?~Åê*RwL?™obÂB‹?™Àò~ߊy?"D³Uƒ?ïK¹ÚÔò?"ÃßvÖø?HöÀ´•s¼?VŠè™.xÏ?•ÁŸØ
?"ÃúC?í7ñbS'D?œ™Þ¸ž'?‡¢¥ÁÃ8'?äVØ°·4?³L 5+É?™™Ë¡*}?ìÎ[™Ï'?¡ÇÓ[N?bSœÀò?U‡ši†™?¸üè=)ò÷? óôPÉ"t4FGL J0507.4-3346¿ß#0Ÿb¹çÀA¦
á'6À:˜CÖ¥éÀ<'">iƒ@ ÈôíÓ,¸?ü¸<ÿ?½
uyÔ­A?å›G;]?ÓwE|Y@ãòóýé$¿îY»È˜Š¦?Ñ*²Æ'Ii¿ÚˆüéJ1¿Þf*]㋿ÐGòká%¿Õ¯?ˆ¬ŒAGNbcu1RXS J050727.6-334628?ïw7B/Ç|?"×çq«ª?L÷euˆ?BžŽ"8›?9Ãäà?"i÷¿"Q?ï‹g† ï?Ž	'Í¡&?0ÿ¸€—Ð?@9ˆÊ»H?Œ¡¬ "¿-?|ãd©)?íøJ¥–?'I{)ú´?utœU™
¯?ií QYe1?­ÌÂ%K5?*3ò@¨?îê©Bä¾?0Aòmr?UÚùnnª?I8æñrkú? ¦–`^Cº?€ùՐÕÈÚ4FGL J0507.7-6104?îúǺqÞóÀAû‰?¯BxÀ9Ry§‹Ê¤À<¡V&}B@Ä*m @ö‡{‰ä?°ÅÜ~ײ•?²=Âno@@}ü…!=@ü!3Vn¢¿âMQâ É¿âò#žjº¿ç¤Ç+£¿åíuÿ‹í¿è˜b—¤ÌÔ¿ïÿÅ}M2¹AGNfsrq3FGL J0507.1-6102PMN J0507-6104?ïÞ´öAU?žUQü-?QJ7äêÅè?"óh¾4{?h¥í}IGÝ?"âi,"uP?𢡄ìjÈ?…šÆ:k[s?@¸;â?WX4éêÌ?"ÔäLŠ!?"‰=)Ìy?ï.>‹¹f?°Ù´?l™/Ó-þ?b˜<å\Ȍ?–¥•­?ÜÉF"?ï¢ÄQfñ?s3t¯¤å?g4*ñ¼Ò?VE uÈ?‡^²)Ô5?ql¬ÀÌ¶4FGL J0507.9+4647¿å•Ykߪ©@vÊa¸¼À:	ÅDBO0À;I%Ü3@ú¦‡é˜à@á~4¹E?ÑÚØÞÓàg?ØÑÐAÌS*@准qž©@_Êe"Yi?£Pª"¹ús¿ã¹%¨05¿ä`‰þ#r¿éÿ}Ž¡¿ï÷x§±ŠQ¿ì)	ä…P6AGNbcuTXS 0503+466?²áËàö?©¹,!,¹?›¤ƒ)ˆ?•Krs­†_?ìàã'j´
?®1eoÁr ?ÓK"^É?Æ €Lº0?¶ô'ëð?·çÀI
ë/?ã{°;üó?ÇOÜםHÚ?ÐÁëTŽë?¨§ÓóÀ,§?ÃÑN͏Ö?£9q֔ÅÌ?ãKW–?¯n¥\?Ê¢ã­ý¹¼?¯Si¬E7?¤ëøcÄ8?êŽ8	¬?臎DP.?±ç[¦P¯4FGL J0507.9+6737?è*M±í+@/ÉèPðÀ8vÖFÉ-À;›òâáH@!Š¿¨X¤?øž¥Ýtº½?ŸL¬^ ÒÑ? qÇÿ™¹á@ÔæŸê%@áY¡±ì?ïy¼NÐG¬?']$É8¿ÚþÜÇÔ¿Ë`À	Dø-¿Ð'¦ÂÌÊWƒ_—±AGNbll3FGL J0508.0+67361ES 0502+675?ï Ö"9¤"?ˆîG~ª?Câ&%î\?HŸQHÍÀ?†Œ<E(Ã?ˆ=äÖ»
?ï'*'+…?ˆé½•¥b?NgþY_÷?]¦²T˜¸?‰ŽöOˆ»É?‡Ù£¨³?í2~Ûv?£€Á§¡r?so³á?rA/j›Ç¨?¶ k-÷bc?£¶kDåM?Hâé?Ž'í||¼f?tKÜÇÅÁ?hŠ"z[?£]/ïæ˜À?Œ`u{œ÷â4FGL J0508.2-1937?ëŠï®µÀ?2×@ÄnÀ;*í"1{À<µrþ$]­@xC¬':×@åPäôá¿?Êú8À»Çl?ØHC{)ìã@C"¡@µÚ,†Æ®¿ïÝ7~ŽÒ?ïÔ£"`š¿àé.AÜÄ<¿åºðáÿäÒ¿íøwÀ«×4¿ïÿý±q&´AGNfsrq3FGL J0508.2-1936PMN J0508-1936?ï
¼ÚÙu¨?'ÌþøO?‡Þ`uÿ¥Ÿ?…IPðš"â?'Y4iÑx2?‰k¡ša¬?íq¾Ïý€&?±´Ñ·VŸ?ŒÆ½WGµš?ž_øáÍî"?°Ù1Õ+?¬ Ýž-?é>=±9Ζ?©z²Þ+9?¶‡x6 ̉?Á}v2?¿†š@¾Ã? UÌÿ	ã½?í/¾–ßÎ?—ˆ€_Â?¢''ÞgŒ¤?ŽLfû9?ªØ*vf?Žùÿù$<4FGL J0508.2+5211?íû €~@5#ŸAyGÀ:ÀÞ­ŸàÛÀ<4p¿…¼m@ 
z?â@I´˜c9?Ō[ØîÄ?¨ÉÀ°3å?äù]ÿºŠÖ@mà0ù¥?é"ó1»cï?ïøø²<(¿Õð¡¾+IZ¿æ
gAؒ~¿ç®±Ž'å"?·ôƐó'ÄAGNbcuNVSS J050809+521256?ëNÉázr?´è3"ÜÜÍ?p«Hß¡Y{?s&,僘?Â?~3Ãn?´ÝÁIx^?èyµ¿Nqš?ÆÒŽú-?míëF6!`?‹9{#ÁT,?Í¡qU­a?ƖÍCîÃÄ?êKcä	
?£²«å*u€?ŽíҒi±?yF9³:^?Äñ!'²¥`?¢–ôvý®«?íÂäf–
?•v0ì.ôQ?…¾~SSýÌ?x§èÄn?®bÊW•?"¶)4ºS›4FGL J0509.1+1943?â¨)ƒ Í¯À'ý¼#1]pÀ:	ã<zڒÀ;Ÿæ·Yž@E	¬§@†'QúŸ?Ο¹ï$'?¸F7qÜ;U?èì&>ƒ@ícíbt¿êÁ¢Âi¿ÝXl¾U¼¿ècya•Ç'¿èêŒeÔp/¿ïû'Á^Á?ÐC	Ÿ»òŠAGNbcuTXS 0506+196?í'zŠh?<?°Œ¬‹éjœ?f—úg]w?c,è Çm?²·kكm?°]?;>?íÍzÄ¡ZÉ?¶)ž½ÿ$?mh!®,?{X—1€°?°§¾™ç¹"?µc¤2Z'?ão³<Ã|?°(ˆ¢½z?¬Ia;}2­?'ˆ&(–?՗m_
³?®3C¸3Ç?ìà>üÊ#?¡Æ÷Ğàd?z/m&tx??iDÌ 'J<?·\/5²g\?¡Vír>Â4FGL J0509.2+5550¿ïÎ"þæ-@"Ÿhß½jYÀ:.¶ÁȍÀ<~'­N@;2'D"@˜<ÿ?ÅùԂM͓?¿í½‡?ù7ýÒÿõ@<!í%?ÞþáEª¯¿×*&ʺϿå$u*Nˆ#¿ÜÞ硺Or¿ç¶?A´U¿ïþ±`à•'AGNbcuGB6 J0509+5546?ßjw=:K3?Â-¿ù"y?'›"l
?ˆòؤ«ê?ß{×@œÞ?Âgµl-~ý?ㅈ\Ÿ?Ç֘6?ôÝTæ'?'O#õ?×õH_Œ?ÇZ€•ð|Ñ?åd7¿É'›?±,óë;º?¤+ëõ´àv?Šº€ùò÷?Ò²¶^»?¯°êä—?çÅ
ܛ ?žO÷š|'Ü?¡cŒ§Ä}0?°[Â^{Ô?̒èfœr3?Îùô[4FGL J0509.3-2917?áu…tï	À@ïßã*dÀ;	üȽÀ<»ÃlѺr@ùeä@|ÍT¤?ǼƒDÃ~¿n$M$;—²?¬fóªNN?þ‰ð¯*%¿ì–ŸV¿ÑΗÝ×·¿æ
|?ì¿Þ;	ÛØ¿à8èê9Å¿ïó/lÕqAGNbcuNVSS J050927-291339?מּ_>ÊI?}[ à ü?CÄÜ5Vû¤?9­ÞiÞY¸?ƒ"l÷þ?|¹¸6"Ø"?ïVMÂz@?•‡Áfº®?CŹŸ{?WG·&'5}?"˜Êë|?•iʨ¥‡?î²¹H@?ŽÁª¡Ç?~ÅɊ[©d?nï­H
PÕ?ªŒ:0ŠŸ?Šûö!~_?ïv"ð
Kk?u%a¢¦w¾?\àd=§²?N
Fôl?Ž¿0%o¹?tA`Z{ŽW4FGL J0509.4+1012¿îì"ÑÍMâÀ1>°ÙQ?ŽÀ9YµÂÅÀ;î:Ç|*ô@s·ìj÷Æ@×~¶ß%?³<ƒd?¹1¨C«{n@:$¾ü*@Š_[^?ïû‹[é4â¿àAR—M¿ædÊðSº'¿æ†Å~ð¡¿ç'uÞ©¿çBž
A¢bAGNfsrq3FGL J0509.3+1012PKS 0506+101?ïØ0z"¼Ä?kÁŽüº.®?58Ô´•Å?.›ùÓà	u?r•ÿ(VSŒ?kTÍ,?ïÃü¯6Ã
?'ÉFš2(q?5aín×þâ?Jq6ÉK™ë?|«‰°ú•?ý‡vï'?îèF-Ü$?"~˜÷éo¦?sôØN$$m?dx®üú°?ú0öÒ^?' \á?°'?ïBM–aŠT?y¨ôóaðs?k˜‹a(É]?Upþ‡€µ?"C;Ç©œi?w¾aq˜ä4FGL J0509.4+0542?êP1Š€fÀ3¡zÌNøŒÀ7K(û¡ÌnÀ:î
N@êÙð¡¾+?ÿîȺïT·?–~1xï?ªŸþ…+£@H×°´h@'í~<Q¿Á@WH'>V¿Û R›X`"¿âÚ>û=y¿ß,J
æ
¿å#ªß½s¿áͽ¸‡ÆAGNbll3FGL J0509.4+0541TXS 0506+056?ïéQLù?ƒûV©Ïá?A+?اí!??PcYôrN?‹r÷¯N?ƒ¹KLŒ?ï㦕;?|†e»™?7­ß'S-Ð?LDòdI-s?w+O/Û?{pÒì#~?íw7Õ¬)‡?¢Ü'äKÁM?†X‡˜?võ¾Œ¸?±…VA» Ð?¡w«R˜Õ"?ïçéoØë?X­¨dŠ?0†îº»ì?éUÏ-`?gMY?XFwMã®4FGL J0509.6+8425¿îA‰Å¨ã@8ŸB»früÀ:ö,ÂãÀ<‹2§òø±@Ö ‰ÍÉ¢@`ù$C¬'?Å^I·Y¿³árÌ%]?ìá¼]"Ùç@ËîX^¼?ïúwàŒGL¿ç³ï†¿é¯Pð³[â¿ãƁŽàØó¿ð?ðAGNbllS5 0454+84?ïÄÐ%z"?¬'
m	µ?kêé´nÔM?‰ùP¼¿??oDþ&â?¥Ç<0Ï3'?íÛOˆhÜÿ?³í-Éd³n?‰«ª õ?£§ÕUd%?«àñ4ëÆ?­^*'`c?ív 	æ'm?"¨š~µ7®?`ð{d±Á?€H`À'V¢?°bá¡b.Q?QsN}?îÛ»ý–û?Œ¸	áô"?…E˜=?yÎ[O‹í$?š݁YS?†¬ÞÆK–4FGL J0509.6-0402¿î!kNqlÀ8k™¡ýjÀ:'Ò¬áÀ<ZÆã~¿ù@ &|'²wa@h_dêed?Áb¥üÿD™¿'=<Ÿ/?ÒïœePç¤@"‡®‹?ï÷z>Š¿ã8Õ3£›¿çdú Å‡ß¿Ö—-ƒ›Ö`¿ßÖ­3ªQ¿Þ³Ë>WS¤AGNbll3FGL J0509.7-04001H 0506-039?ï<ï'@®?P§ÀÕwð?XýÏÎR]?QTqõtù"?–Ò<oû?nZòm`-?ï@ÐA¹L?´Õڇc?Q™ðÊõ?`PœÄ""¹?–ë<X¼'?&õ"º?퍟lOÎ?—MiÅ2î?wSGd e?b¿™]tL?²Ð'>Dž?–«'—ù?í†FoP´?'út«æÄ?uU$¶§o~?b¥úüiÃA?¶{f?"áSb_Ê4FGL J0509.9-6417¿â"ÄoÀA˜>}QÀ:N°÷"0|À<"ê"]ðv@ Eúأŗ?þ-Aª?µ¾ S¿ƒ'ëÆ&d?Ð`¼ÃÀ3·@	Ý
$¿á¨†Ò¸©¿ã·S½v¿à*®"Óa<¿Ù‹z‡…šß¿ÚoUã·J¿ÜM8'}sHAGNbcu3FGL J0509.7-6418RBS 0625?ïÐç$}¤?—PäPpxþ?4s…£¥?Hˆöœe)?vJÌzCӜ?–ã2\\?ï²\SÖ­?"P|uUé?'#Çóa£ª?@'>Aöˆ?ƒ[ê‡5?ƒêþóˆ0?ï,ޑ¾ââ?Ì&ٚZ?`mïô¢´Þ?NŸîHÈÐ?˜VoɏMC?}úΞ…E7?ïÿÍ_?q5³´?C˜á÷Š­?2`Hùc å?ŠÆ~ˆÀÜ\?pöx%Î+ó4FGL J0510.0+1800¿êÈÛ?pÀ)p—AЅÀ7÷uôxãAÀ;F­)¬@žp•@­@ÅÂíP?žs_Yhj?·«#Ú¥¨q@]¢r†/@xkv›"?¡ˆeûÖ~¿às-õÐú¿âKL.¬»µ¿â']ÂS¿æâZh+b"¿ê½4D«+AGNfsrq3FGL J0510.0+1802PKS 0507+17?ï¬z{¡ìû?xA{—b"Q?@¯ÀÝåM;?9ÙOé%ê?ƒÖe	¦l°?w¢1øô?ïËÀú-ÆY?ˆfíl+iJ?4؅Dh›4?VŽ`à¥bW?xÑú"ÖJ¶?ˆ,MÿX?îî²RŒm?'zšSÏÌ?…úŠ´Ûàu?…0SàX/w?—,pT'-?‡X	¯"?ïßM¸(ª?]¹¸N[w??~ÿØÄk?D–"®?o¶O÷ȏ¶?]H	1=â
4FGL J0510.4-1809?å­>kÀ>05z5PDÀ:¢ÏîÀ<œÀ<uªŠ'¥a@%ònZ@5ÚBU?DZ¼»‡«?ÀêB> ?ôE;ÞÓ_Ž@
åð¦p‹¿àsco;!>¿×!˜ r¼5¿èà<K	鎿çŸÌäu¿ãC‡^ƒ˜ü¿ïÿšÏúAGNbcuCRATES J051015.50-181227.8?ﺳ¥'ëÛ?|Ú²¤+?P<¹†#¯Þ?m zaŸò+?~–þÝ&›?x]£^¡&?ï¢ü0y«§?ƒÊ1æ_¸S?4áV‹6?N™, 'Ö?†™é-;e±?ƒ3+Ñ6ÍR?îåTŸkL3?… þ}å™d?p¼Q8ý%H?d·ë÷ \Æ?Ÿ&WÄW0J?ƒÚÃÀr?ï±+ ƒ
?g[R:…c<?K»Ý/?:;î÷¹?ù{vjq?f¡ïÃQ4FGL J0511.4-6804¿åX…à19ÀA%×ý'w>À:Ï&رÝÀ<.šLGp@p¦d]þ@ºV€?U€?ÅãæÄŗN¿mÜ^y?¡'G=VM@'º¹Në ?ð¿èZ,fWѿ듦¹Ù«¿ß|"¦Ò¿ÒŒ\š4Ê¿ïø×aütAGNbcuPMN J0511-6806?ï?•v÷?•ä4µWp«?:5Á
Â/~?<±<ò?>?‹^lš#°¾?•ªµ¥¿uâ?ïS.W·†?"I`õV#?LýuÚí9U?h)"€ïpz?"²Q&1¥†?'¹Ø$^?íwÕ<Õ³[?ž¶[W=Å?p89àM^?eW•"z$?³?ò•´`R?È,¼6äà?î–cž‡??ˆËi¦Íq?J%™³9~?A'7\ô/?¦/…‰ ¿!?ˆ¢÷Fë<™4FGL J0512.8+4041¿ïÿúfþ†?íJf@%ßãÀ9N™û¿(ŸÀ;Å(wŽ'@0—²Ž³@TZDïô?µØJÀ~Æì?©ÚˆÍ¢
?ñËÏÇSH@Ñá»Fg˜?É"üÚ0¹¿ç¡Ìþ¿á¹	ÁŸÈ¿åF]É^ٿ༰À&Ì¿ìaU_Ø؟AGNbcu3FGL J0512.9+4038B3 0509+406?î5:^xUN?¦·rž?Y?Zßæ
‰s?XC5ÏáO¦?«ÕZè*Ë?¥‰ÄußÛ?ëÂ!+¼®—?Æ#/]*
?[ïIá±K?'ë°Œ¦s.?ÀÁAry'>?Æ
~ù>?íGðq@ø?˜€åx"Jõ?'l
¯"d??r»}—úSù?³rýæ…k»?—-Å8·ä?îõ‡ÎùwT?æÉ&©›N?`¡9y* ú?J¸>ßåÅ?Ÿ:Þñ«Ñš?j3¸Àô4FGL J0513.9-3746¿ï¼ÜôQÀA[¾<Q‡À:ûÏ[óEÝÀ<~>TÏe.@)aIñæ@>"DÎf*?ÕzOÇã?ÞóÞ>d>Ä?ü4E]c@3ÝKue?îñïÁ™gð¿ÂtlùÓk"¿å6Aü$¿ïÿî—ø¯ª?ïþ{¿ïÿ7Mt'AGNbllNVSS J051404-374607?ï‹=»fåY?<Ï)‡ä?h8/'"M?j³0r ý?‡"iÚbEQ?ŒÔYM¿‹-?íÑ:ÐÏÑÌ?µàÙ)yí?…š'œìÂÌ?œÝ	È̬í?­…ÉDz©?°ä"ÊD"?êÜQÖҊ?£mFJ=˜?«x\nJ#³?"ðdä'ó<?»c§:$YÑ?œ&…NÄRÁ?îñ@Šm^‹?—8'r.½?K/gçI€ò?W"þ›tÿ? 9¹Œñc?—U…á4FGL J0514.5+6247¿èŠOXûN@+š™0¾
íÀ:£>ºOò‡À<uÌÿøsD@µø/°@"EœÂC?ÂnʸöV3?»ñ'Ž»F?ú|ÌQ#ß@€ýêQ¿æj8î^
?ìšÏú¿äW­Ñ_Å¿ÜXGŸ{ÛÄ¿â^zd¿ãœg¿¬Ó³AGNbcuGB6 J0514+6244?ïHó'Öe‰?˜¡Â,!¾?]Ü`¿±'
?bK¯Qy¦Ý?•Ôù85³?˜\÷€áŒ?ïeêPäö0?"oۂç5&?QVSõþl-?]?<·ãæ?'-P¤Sa?'‡uˆËl?î³/w ?ÙtéG8?oh'z.Ï'?cæÿň90?¢×³ç•¡?‹Æv4oµ?îrÓ»"ƒ?ƒæ³…Ð?'ÕP'ªæÇ?mÂ\g{Ÿ?¤)~Ÿ›þ?ƒ1>
¼µn4FGL J0515.5-0125¿ÆÔQ˔À5â]B¡À:š¶ŽœæUÀ<^@îݘÍ@s–ñ?ùüÜÊpÑú?ÔKa}H€!?Ô.á_+Â?þl˜å>³š@‹ö~•?ïû¢}˜Ý¿è¯L¾õsµ¿á§?¿³‰°¿ÒÇÜ£¦¿åŽé<o¿æÞÛB0|AGNbcu3FGL J0515.5-0123NVSS J051536-012427?í•Dí‰|?¨'Z Äà?kàdVx?cOn:˜sß?²|ÿ¼´Ql?§šØ×bÜ?ïn.!ù ?˜Äˁ"ýõ?bÃééPcX?q¦DíÕ?œù¼þ–Ïy?—[í[ÇP?ë|­pŒÙ?£Ú,Oô;?™²ùÏY!:?Š´&áÊ?½­Ù(¥Pï?¡W:©ï?ì7JÆ`3"?˜SmÓÒIY?rq¡}!‰?dÚ~˜ü
?½»F'P?—í"0ézl4FGL J0515.6-4556?íeQ"LèÀA°K	éÎÀ8Äb\ìj!À;ý'æ÷ñ@ƒ)[Cµ@%AÁÇ?§´Èbô…½?©»Ôàu(Õ@$x]ï"@ØëpR#?!HW»0¿áÜ_|gY«¿æL8½¶¯¿äR½ú¡ò¿éwomv% ¿ëQ­DqIAGNfsrq3FGL J0515.3-4557PKS 0514-459?ïÕîޙ¡\?q®Ò⮘??ÅxŠê&?8w܄ëI2?s9'£&?qäŸ{Ò?ïÕË[5€¬?wjD²x»?'pÁõHO?=îwÃôl?tbß/ÿ³?vÖ¶˜G'?ï#×—I?…óGžA¼?oaÆLK?cëÖùæŠh?™OS#c?ƒ¨ø9s?ïü!¤³¦?1ó5JÍ¿š?v¬þ·G?Ý]yÈjæ?:Õ/'"þ—?0†k‡ïV4FGL J0515.8+1527?æ;‰Ö­÷À*!ÅXdEÀ8ådÍßòCÀ;¶_"ÊÕ|@ É®ŠA?ýµØy©9J?®èO_8Ê¢?´ß="u@ÇiÃèø|@
¸÷f©WR¿ç8ôõ
¿Ø¨ÆÞ \A¿Øc¾ÁF[Ú¿ÝbßÆú{¿áÚaàŨ¿×¥Â¼þx–AGNbll3FGL J0515.8+1526GB6 J0515+1527?ïì쳺¿?X(ç^•–?1z›Ü|ãÃ?(Ž‡Í›?aϿе¤£?V¥Iƒü€Ó?﵄`Êú?†úø‡?B(ù8ÞH?XÊ-$UÁ?|kOÙ³[?…ó¾)wPã?îŔŒñ"õ?'3Ý5 HË?r³lJ²t?q›E|S¬?¡PI®äzg?ŽÂð3¶i?îZŒmŽ5Î?Š€¦È~?r_8® ¸È?]ŠobÎwÃ?¨RHŒ?‰X1âßø™4FGL J0515.9+0537¿€–=¶pGAÀ2Iâ%úeŒÀ:÷ÒîNý"À<AÍ¡Þâ@Sõ±G‹/@'l6Kì?ÓaŽºú½¿",ß5N?ÂgBÚE0a?û»‡ëqR©¿å;66ó²¿å_"û-¿ã4íþÖ	¿àŸ=è˜Û.¿ã€´ÆEÊ¿ïê¶YFmAGNbcuTXS 0513+054?îÉ(蚥?—Øڏ"ƒÉ?UnãÍÓ?O''HŸ(?¢Âƒ
Îü?—V"j£<Æ?îñ¬6ƒ1¸?ŸòYŸIt…?]g4tߒk?vó4¡áÜ?ŸôèKÐ?žfx¿«>?íkñkëêx?–¿9ÓX%ý?'~<U?s—š²µ°F?²`Ù:'?"ifC†Öõ?ì,'ªÀ×?,>¶ÄM?iX؂ $ü?^µvœÀ×Ï?½Ð£çàø(?*ÿp‰‹s4FGL J0516.1-7240?Ó|T…¤€dÀ@kè^9qÀ:gÝDUGÀ<2Ô\.Õ@|<uQ:Û@ü
éÿ
?Ãw©Å5Ô£?³'Þ
øø?ðG™ò"í?þ.zœ~Ph¿â5N`¶#=¿çv-NäH¿ç|U†DR?¿è@¦¹<Í¿ïÉéÍ³}¿ï	AÈ!laAGNbcuPKS 0517-726?íÓ¤>Ëx?¨Q£¶ô?3WяGå?w[ø'Èý/?®èŠÁá_‰?§1©L4Ï?í("'ÂÐ?±V…™a
?…|§¥Ì`?Ž…ãOøAˆ?´QÍ/ñ?¯²Ïc;?ìØ!ÆhúÚ?œØƒC9í?'Vß.:]?lS^?´žœ욡?˜AR=`W?ë]¾ãßÊ'? ÆVæK…@?¢;pãq?Žñ
[jz?»ôH(ø=	?ÔTx‡°4FGL J0516.4+7350?í~"$Ï1@3Åf'|EÌÀ:~…AÀ<uV=ú6'@ I«w?ü΍+Í
d?¶{iضºè?°õØ^ÑF¯?ù-6´Çó?øòuJ×?ïÿ2z¦K¿çiÊ¿+y€¿Ï¡ªŠ,¿¿Ü=›{?¼¿Ý ¡€mΐ¿àÚÞrç~)AGNbll3FGL J0516.3+7351GB6 J0516+7350?ï˜$³Áäå?€'ܙÐ?Rë•4R[Ñ?KÕG^8–?‡™`hü{?5çÑÈj?ì֐Ç|¢Ó?²©šN‡Ø?"`$×sL#?™Ú'þ‹?´spŽ>X?°½€¬Éq?íaKþ[??—<c5ÝÁü?"k×&y?t¹ë¹W|4?²jÅ+a.?•ùqÚó?é©Ï
#©?¡KÜ®–Q4?­â`¦Kœ?'ºû/sç??Áà+ªD©³?2ôÁ°£ 4FGL J0516.7-6207?Í y'W'ÀAaÅ.rÚÀ8šq
"=À;Àâf'@·ut@Ù ¡`7?¢[_LA?¨'K‰Á4@!Àoz@h²ŠMÈ?àÀgc¼gû¿ß}¡ku¿ãŽ¶aP|ð¿à˜ö«:¬¿æ䁦ާ¿åó
ƒç€­AGNbll3FGL J0516.7-6207PKS 0516-621?ïÍ
ƒ´@?m&Íwm¤?1Æ6ïËu+?''¾ó\±?x\Ú¶ã<B?l_5¢Óü?ïÀµWˆü?€	
è?0µ3+çö?BÝB†Ï_?~šFý?!EÝB@'?ï,
ôs?'>mGDo+?nïß«K¿š?e{EZÁMN?–žb¬%S?~üݙ:$?ïã¨RòY?U"®~®½?5×(ˆ…o¬?'ß;2Î7?iœÈíüøW?T\°
Ò+4FGL J0516.8-0509?æRʊɼÀ7YfYÑ,®À:`œøÉ«À;÷À¬-@ÆÎi/œ@C¼Œã©?ÇÝCýÛ¸x?Ù)x¸.@H/yjO)@	†qÀ?ÆxÌ$ý»¿ãu"FK=ì¿ê{>º¥Ù¿îÞwëÉè¿ïÿ¤?åÉ?æ2ËŸAGNbcuPMN J0517-0520?ïnþŒƒž+?'"uoÔîÒ?s‰Ý?w8$îár?ŠHŽÚÈ°9?‹ëÑ]O;ˆ?픏2–¸µ?¬Ãµ{ö$D?'"cµ,üi?›bð	×?­mZûýöp?¥Å½áP?éÁûè¶"?¨ÝS‰hT?®ÿ›>K?˜
òE9ßj?Á:H"µ?£ßPYƒ§G?íƒÄè2¯™?™ñµ{p[5?ŒM¯,âæ?x3?ܟ©?°X"ØÚFÕ?—·¤ÀȒ±4FGL J0517.5+0858?×)ùë¥À01w…r›(À;e DC%ïÀ<ì&qƒÐÚ@!F€ÞaÊ ?ý痾Ή?Û
úD5ë?ïÿÜ>Y×ã@ÝK 'ß@M T3^¿évá]ÓoÔ¿îí0º²îÕ?àÖýr‡?¹¸ÁÝõ-¿ê²÷¤ëá¿ï÷ÇLZK¦AGNfsrq3FGL J0517.5+0902PMN J0517+0858?ë=f† å?¾yqlŸ?©ÂŠ}–&?ªq,õ€r¼?¹6‡ŒÿîÌ?·ÁŠs°Ó¬?æ{€8µ'?Ï0fã";%?È	'îWeË?Ë=FO|×e?¿i!‹‹5?Ào©ÌÌ?è_'IÁ,ê?®Ó¤Wï?³¹ú£2'€?œ….²¦?Ĥ¹‡b?ªäÞÇ/'»?âéùÿµ?ÂL$þ÷R?ÊiÎ\¸rO?¿±˜–ë¤æ?ÉñÑ»K:ß?¹^Y`Uâ4FGL J0517.7-1758?óâ)À<ƒ…@FA-À;SPßìdÀ<n"d¦rÆ@ÙZ.Ÿ¦@?û˜'3?ÓààHŠ?èö'¤‰·¤@
;&wºL@JE)B¿àÔMà½?½t˜j¾e¿ã«Þj®õ¿îwàmò¿³Ï?Bàû-¿ïÿÂ"NßaAGNbcuPMN J0517-1756?îDv'_?±÷S…6ÒÛ?rµÝºÀ?'ëPÑ?¤b[kŒ+?¯TÈeÃØÜ?ìòÈÂÆF?¹pû£SáL?˜·.¡?©fpÙ÷"Ÿ?²=M®h†ô?±•<M, ?êH'hAÑ?¨ ùÝÉ6?®¶läÍä?šP=׃ùg?¾cíWh?¢_^ˆOæ¿?í"
	ó¹?œn˜1•ºx?‡þš"ôV?'W•Í¤è*?°gܗ/ã¬?šf}©ù4FGL J0519.0+0851?äZ6¤¤1À/ß-@ªëÀ9:2áԛÎÀ; ˆp|iÞ@ûPæ¢`è@Œz¤áÌ8?¹óô®é?Éme^(ªC@h@µKü­»?Ез=¿áIéXÎG¿èÐn**¿èƇ~9ö¿íÕç]qË?¤7ÀvõAGNbcu3FGL J0519.5+0852TXS 0516+087?à—Ü#s¤®?ãVqýj¢?ÇÔÚõªö?¸ýä3•þ?ÒåÚ>C;¡?Á)?ôôzë?æð_7îz4?ʹFd—©?Æ©÷Dь?Æ_U&æ¥D?¼e²R‹R?¶ª¡¶°%?ã~çæ&?²®öGÏe?Àr¦FÄÜE?¤.<rüÙ?ÐÈÝ›Ež?­Ç䨱‡ ?èg—Š[½?©º+£Ëòp?²»Ë«ö?—>c¶w¬?ÆX|Ô;?§Š}™È4FGL J0519.6+2744¿×ô ý ÞÀÍW¼w¯À:œŒ" ÚÀ;ætxwàâ@  àBöIÉ?ë6™ŸxÖ«?éýáí›N?æ‰=–c"4?ü"§—‰!@ùQê™¿æT~<Fl¿êöDà"º¿ä)%}½ðç¿Ôr;†¾Ì¿á$ùê<I\¿ïþ«6z'AGNbcu3FGL J0519.3+27464C +27.15?謣¡(á?Á
™ÅßÂ?'	<ú|Äz?}㺷ÚU1?Ì,Ý«¶46?ÀÄÔgÍü?á?Aœlˆã?ÍsY"Ô2?h¹GÇ	ñ?"íΖ恿?ÝP
7˜Ê%?ÍóP¶?åt‹­ÌV?±údçøN?®W}ó,†D?™l,;@^?ÑLó*>֋?°$".d³ñ?éÚíVꖃ?¸p*¹¬|À?(áÊ!aI?<°`Ñ fŠ?ȎB«ãœ?¸oÉACl©4FGL J0519.6-4544?ï4˜H¿?#ÀAUa=1¹¶À:6Ô;VdÀ<~¡ÆŽÅ@QmPæL{@'@œ¨AÓ?·óTKâÿª¾ÜŸ'Íú?ò•ôÿý²?ÿÓqíLa¿ÞÍ–%œ¿éŠŸ䍿æwé`J¿åÌQ¢_¿å4јäh¿ÕV¢ƒÎTAGNrdg3FGL J0519.2-4542Pictor A?îåeëšó?—®hCé?wpÊoËÇ?qª£/Ĥ÷?w*\ð®³?•ƒç4¶»î?îp×Kšþé?¢˜Êđ"?h|ây…	¨?nâ TÀ?§j½·Àá?¡ßã8K0K?ëÊ ­òµz?¢ßBTË?"0{§Oc?˜ÄS²"7?¼âÛÐ@€\? ØK·cÎ?ëÙ½!0™?žÙý.ç"?'ò°Ü;?zäï¶k
×?½ÚóÐ?ž;vfì±®4FGL J0521.3-1734?íû[ؐF×À;Ž~bÜn+À:dál—À<>'(ŒD@¢ÁÙ©ª@É%x_?Á¡??Ûã?ϘiƒQX¸@
Ь¥åØ7?÷\mܧ`W?í´5&Rz ¿¸º¦?Öjì¿å~SEÎ@¿å->â"Þo¿ïÈÇ.¥/¿ïýD™`AGNfsrq3FGL J0521.4-1740TXS 0519-176?åäŒVF<t?ÃTûÛÑQ?ÁŠ›«eF?¶-bIÑ?Æã2ûÈ?¼ì4a[LC?áLklö¡?ȤúÛ(%ô?ÐƶnùÏx?ÆKèI£O?É@ån4?¹MokêW˜?ä‰ÆÝÂÒñ?³
ŒD™ç?ÄÖ-Dz?ª6'ÖÌ\?ÉÖ[-/?¥ñe=1W?Ùhêì v?¬O¿H[j"?Õ¾¬GŒ­?²¯¸ÖÜ*?ÐØigËÒÜ?©.ñ2ù4FGL J0521.6+0103?ï2êÿÎèíÀ3Zº8u'SÀ:ŽbwÄ\¼À<]Ú{9@ IKèá«V?ÿÉÉã
?ÀSÒ:
²?–8…‹"f?Ùât¿D£ô@$3"¸¿ï㸌íº?ïÿº*2Ùq¿åò³{Âîý¿ßEœVã;¤¿Òê"ޥȿá1ªlÞAGNbll3FGL J0521.7+0103NVSS J052140+010257?ïôø'J›<?Pc'œ¶áú?$cÈï
P?ùҎS–V?S'dLå¤{?O€?T
ô?ïΠ–‹?{ÆCJÃ#%? ؄h—?3ê–ØÖ+?x(ðÖìõ^?{>G"fa/?î彌–=d?†Ù]=#ù?b«0r/D?QBBì? yt/y9?†>©"zúš?ï•$w|é?nìówëÚ$?LXÃs¹Ñ'?@Èj­ž'V?ˆöjªå)
?nNn´è4FGL J0521.7+2112?Æw÷cçÀ!iÓpóˆÀ6Þ¯\y}šÀ:­ò<ÈÞ+@]"ÿ‰b•?ýžøé‹Iu?'œÅ+	?§v™[ӇÉ@Çxþï^È@ȅ%ï'쿍4ö`€/¿ÙÇCáVF´¿ßûÛÙ>¿Û[$^.3š¿áø"ÁEZ'¿ÙÈý4s¥AGNbll3FGL J0521.7+2113TXS 0518+211?ì¯`³ÚÌ?¯ðI¡ãS?Zt—7ˆX«?VŽ{öƒ?º(K~?¯¬†'ü"4?ï
E{S"?ª!@tx7?Km}ˆÚÏ?e¨5U3¹?Ûä©Tël?©ÏQ†òO<?êOÿFç"?¬®@Ù~É?ŽS|‹XÜb?"TúYg+?ÄÚË®î?«uÉ¢íl2?ïÈ3KW)?néòLÉ©O?'?BÛ`0x?!y]âd?{,`=¡éì?nµ[š"4FGL J0521.8-3848¿Äq߉=À@®1¤½º
À9ò÷Ãñ[øÀ<Yñ›@T¹³?ˆ@"C'OH=?·1NA+™a?©v(ù!?íºôB\›â@'̳¢Y\¿]kW´>W÷¿åÔ"°Õ¿ê1"ÝIó¿ä\¢b•÷N¿ätSŸx"¿ïü¿øÓçAGNbcu3FGL J0521.9-3847PKS 0520-388?ïíÊßÍ
ã?}½—û|Ö?6»ßdÓ<?Og%'Ñ«?^»}n"?y>ù¸0?ïÓpƎÑ#?zÍ[C6è_?$šuǾÎ?LS1¯}?u¢É
^ٜ?xã'ÏñÉW?ïB$͏X?|Õ{âú¨Ï?g	LJ—?Uuø]"'¨?"×»]2W?z}ŽŽÞ@¦?ïïÜ|'J‰?I^_'gN?-h̓è?§£póy?\—¯Ñ[?Gµxê¶.4FGL J0522.9-3628¿Ò›í±É¼À@\] l‡À7Ÿmži3À;¦¾Ë'Iò@ðáºÅŽ@øÛÎÈO?"¸ý?¹Üä?³v¸îôiõ@ôAÿ~Ñ@U9˜R¿Ñèb8Yc¿â|Ê@€x¶¿ç°c	º"å¿çJ0i¿çäGbj-p¿át>KëAGNAGN3FGL J0522.9-3628PKS 0521-36?ï±z½ºp)?}*zÌÍ@?Kó®fã+7?EÃ'Gz‰-?âªõÂ×?| qrÖp?ï—Y¾ðŸ?"ïá	 nû?A=:¤?Q5"%ÀÔ?‰'"j?"Å#»û¹?ï*ڃ£˜O?ˆÜX¼yº?u"ÂÉñ|þ?u_Þsâ¼ö?•?¾Ù–Ú?†­ŠáÃL?ïöÞœÍy?C7ùQF?/´šÒòî?(©õ[";?LšnØ
š£?@ÑfK%4ƒ4FGL J0524.5+2839¿ÍÂ+Lùœ¨À*Éòý¸þÀ9€ŽÌܽÀ;âF¼|ó@ X#8lÄ?þV>¶4ž?»àçáÑ?º ïZP?ÿ¨Ec·_}@ {KÆÓ?ì½q +Y¿â¾È'«hÏ¿ÛþcEÿڕVß	æ3¿ä;uÂ#ü_¿ØåÑëð~ƒAGNbcu3FGL J0524.4+2839NVSS J052429+283918?çL˜üáOv?³¯Ë'q…ÿ?'\&
ç?u4ãÇï?ÐÓí•ñØ?³Œà«N&?ڐœl c?ÄÌQ´‰½$?~ã!iº ¥?…Õ鮖±?ây뇎?ÄÀKl½ñ?è+‰ªˆá"?¨(¨æ`?™öB}L?àtXú{?Ì0:"4*?¦ZÀÜLE?å‹u¬ÅB?£4ENÿû?©Š‡Œ;P?‰Çm÷8rÄ?Ѹ†C´î?¢UwµFÇ4FGL J0524.6-2819?à›þNáÑÀ>c…@FA-À;"ƒ°jÀ<Ÿ˜!ÊU#@ˆâÖyt@®ˆ#Oa?ÛmN·ó÷´?̳ɛ"ñi?ðPêÄ.™@
'S6³ÆA?íJa¸¼-¿è3hb?_¿à5B!b¦=¿ë•›¨g'¶¿ïüËÝäw8?ïÈm54?AGNbcuPMN J0524-2818?ï²:OË|î?˜Ad²4&?HsYƒ):?VÉÔi3?c?ét׈'$?—Ü9¶è1|?ïP¤û!õ?™ïϕPîº?Uy¦º?jSæ¥hûõ?"žSÆ;UË?˜Ra¿ýY?í÷"–©fT?•pˆ»ÓÈ9?ˆLB¸|ˆ?Ç²Â™{?ªt¥çgûª?'ÒÎRÀ«?ïÏû'6?eˆloœX?&JkwºV?#UŸyƒÕ'?wP(«]¦—?e:G(÷ú4FGL J0525.4-4600?éjT.wÙùÀ@Öb=ú	À:bøwu'cÀ<dà?p@Ðÿ£ä¡*@'÷
èöÏ?Ãþuf^ƒÄ?©‰¼VÝÝ?ႣžU@#?ÿ·.Lïqè¿á÷ÀBû¨¿è¯•ÿÜſ㲁œøŸ¿à¡?«;®¿êp$ sRˆ¿åÛÍátϋAGNfsrq3FGL J0525.3-4558PKS 0524-460?í2òSu«?¨A³͈?'Hï  9?týè	R?´oJvjH­?§/'+Ô¥J?îñåPÂé?™±"×Oõ:?Zí¨Jüm©?f4>1ž? 
=¼íû?˜q=–Ý~©?íN"Î"?˜4¨Ùnç?ŒmH÷ùž?€'ÎT6ïé?±ý¾:è ?"ûîî—2?îZáû
¹€?Šb‰ïHf`?ƒ*FŠnéÀ?p%<'´
ê?¥‡N¬ˆ­š?‡…زڙ–4FGL J0525.6-2008¿í¸ÌjÒ1À;ŒŸ±À:Ý
s†	šÀ<§Ç'#©R@ÚRý¨â¸?þÎE"I$?Î`ù•WÁ?ЬÞe%ž @vLe3`€@:@ºˆ'¿ïøªñ°²?ïöCže[O¿àdïY­¿ßÏËd—Ú'¿çf½+-«¿ïÿõEq#AGNbcu3FGL J0525.8-2014PMN J0525-2010?ïÐÕ½Ãí_?kfûìŽ
ü?Svž-Z?ID~…˜Ìh?r·y—½ùÅ?hÓñÏ?îCK95?¢â§=
f+?m?ìÃ5ÎÔ?z9²uQu¥?¥*Ìÿ¶?¡DwÀo…?íg…:
?–‰ÐžYo:?"6Ø.Ú½?†–÷
ÌÛ?¯ôk qç?i¨çG?íç&	>?ŽaÎBŸÁõ?Šc\\ž…¸?tG8‡Sì§?ª÷&ˆFº®?Š¡8‡Þ_4FGL J0525.6-6013?Þµð»-À@ïz€Ïž8À9ۍs©ÏÀ<I<4c´Û@ £‹7?ûìUÿø?³Ãê%"N_?¥x¥X>°j?óo Ä0@?oߋì2?î*æþ§:l¿ä2ì@Ûgo¿ÞT"f¬‡¿ÐÍzÝð,¿â•†¢Z2¿¬éÏ£'7AGNbcu3FGL J0525.6-6013SUMSS J052542-601341?ïDGã"F??‰ëYøXíÌ?XcV4Ë?K±ÑãV?•ðÎ8uëj?‰9эW"â?ï"~¢†?•Ô€Ýdf¤?T·öžÂ[õ?^å8°/³?šd¬S"i]?"þ¤<ãn!?íYŒÃ0;?–@yÇ¡¬?SdÙº?qÒA	fË?³
o†Bî?"ž–®'#q?ílÙ·?wÎ?7œ9˜?…ÅŒ A1?pŒ[œ>?±à€Ä9s?Žk‡Œ€Ak4FGL J0525.8-0052¿ê'ÛÖ;F¹À3\‡D,»À9÷Í-DÜ©À<(Y‰QÞ@ÇRŠ¼\@C«Ë]a?À'Xßj3P?Ç¢C÷¦•+@܈皮m@
¯Ò"¢k?ïn¶—b&¿á×]Ÿmn¿ßr5§º¿ßO{hV+¿åýJä)िïñ£µ}AGNbllPMN J0525-0051?ïÄ£Xåñ?rXl‰ßö?gÎ7ƾ?cMŽY?+L?r"lq)¼?g]^üjO?ïú8¯Î?–1•¤i¶?iÎû	¥à¢?xŸüM ·?›&وèJ9?"zŒ֓²?î­O¸fp?Ñ*Æâëú?'oý4€…x?[G¾õ¯? "{·Yw¥?ˆoÙi77¦?붻˜Çï?—…ˆú…3¯?"wN‹""?w"óù­?½,[æ$/V?–X'{'ã«4FGL J0526.1+6318¿áÖæèƗB@.bTæâ!ÉÀ;"®"i›À=u‰ïØk@½"ªú¿ú?þ@ÊËjÍ?Ò¼)œ0¢µ?àÔ}e†l–@
dëVûX@q리§"¿ïÀ	ÿ÷?ïúDÕ&§¿Ì¹¯ä‰¬ç¿Ül±n¢u
¿ïÿ«±Ê?ïön¼v=tAGNbcu3FGL J0526.6+6321GB6 J0526+6317?îŠ 6MÎ?¨Åg2H«¯?™Ej'´*?›g¯•û'«?•»¶®³'Ò?Ÿ>•Q@3?íŠÒP
™"?²jžàÝ"?'™""¶Î? –?Rƒ€?®†IÜŠ?ª"gÁÈ#t?éù¤¤ÊÂ	?©"Ý-ÿö?´,{n(–? Ñþó((?¼®^;Ç? ¾Go£8?"P·?Ž]	V†©Ú?i¼¿ç ¦?~ÏÇp}S?¢¶è?‡•Nl@_4FGL J0526.2-4830¿ëk`Ô´«À@à‰~™cÀ8QÔâEÀ;Œ½vîsç@ðmBùyÔ@Ï7ûïÐ? ¢òˆÉ×?±)¸
Hx@¾å@a @a v­†?°`Úá7'é¿àúõŸSí¾¿äv^½|¿ã–Ð[͆0¿ç»ÙÊâ¿ç^1¾éà.AGNfsrq3FGL J0526.2-4829PKS 0524-485?ïgh!‹µµ?†Ê£sŽÃ?Ef±Ñ??†{¶4o;?'g™Æ?†'ÿċ^·?ïÈÕZÁþ‡?},(•\L?0°¦¼æO?E¹T'w#V?zŠRd"í¥?|uƒ5Jj¹?ï!Jîb2?ˆ¦ª¿j?sl{Ã;69?oü¾XÀ!?–ûƒBêï?…¸PñÓæú?ïé‹u\'?U*TÛvf5?$~¬²­gŽ?B;'ó?e, 2y?T~7EUŽ¹4FGL J0526.3+2246?éJb…oÀÓÅyò4eÀ:bnŠ!WÀ<–C£Ã¿@!›i}r?ÿœ
Ý©"ã?Æ3–ÛNDÜ?°,¡r´?æ"ÿ[•R@$=Pš¿í®,Ε#é¿ì÷iCy¿ÔDhz<Ý¿à- Qn޿嚌Wè¿ÂèL:wJAGNbcu3FGL J0526.4+2247NVSS J052622+224801?ëk[YŸZ?¸M¢äHî»?R"ª9?E'H‰ñœ¡?Â.‡tmT{?¸>¢;Ù?ä]µÝ°Ù?ÆZ1—?MmHMòS¼?c½¸£oé?×5Ý xí$?ÆN»!»í!?êŒäUx¨ù?§Ö§¶w?'vøürx\?nøTqP÷¤?ĤÿV4–?¦£Ãʍï?칃b'?ÝØ"dÔ?bý34?WNŒKUï?¹›þ+¯?ü—«$Š4FGL J0526.7-1519¿àâZ‡NØÀ9~ÓØYÈÉÀ:d)uDÀ<FøE ›@Ý7•B?ýçOšr®?¾öڒ]:?ÁiíˆQ@ÅlC9@֌W¼ªk?ïÿÐ/WÜ`?Ö~?¶N[¿Øò°¡ôó¿àkÑtÒ9ô¿èŸÑâ5iÄ¿ÇE"/_iAGNbcuNVSS J052645-151900?î²Zy ÉH?˜3'Ìÿù1?"£¡I¼‹Q?…[³fÃ'?Ÿbà7'?'Î.Ó¥'?ìÙ¡»,8˜?­ÜP¶0›º?"%-'L¬E?™Z½wö.Â?´)¦Â.?§ÜPÀêÔ¯?ëýDrríŒ? ]Ó	c"?™"È$˜Ø?÷'‰Uà?¹Î7z_mj?›.y²¢ó?éP÷æƧž? iOIß ?­ù×Óu—e?ÿŽ>•¶?Ã=ªpû­?›BÍ­]Ø4FGL J0527.3-6223?°ɟéiÀ@ÀœÜD9À;ÝùzªÁ	À<ý'œüûi@!ûÛ® ?ýç"Ä!?еâlvK?uÁ	þB?°ÌáßGgŒ?òBxåÄë¿ïþ×áÓÅ?ïÿJbú¡¿æk´ÿ{ µ¿Ô…4‡Ç	>¿äŸùš‹1!¿®$æ¿<@xAGNbcuPMN J0527-6225?ïèÄÐ/êQ?co9ªLG?и ±†;?˜3­Ž'‡?f\ª"Ë?cškXùÝ?îœ:fp£Y?¨;É.
ã?`4¢W>z?i£E=ö"?¥9séG?§Ô`·\‡ó?î&«KAã?Žt
IïCÏ?s*¹ŠWç.?p!¨Gúh?«/ô–Ò¡?Œhp¥°?ìŒTó	b?£n€Œëv?‡V%	·?€­]¶Ý»±?¸²›75þ?£ÈÃ
¾—4FGL J0528.7-5920¿á¶5ü¼(»À@ĝàP7PÀ:~Æ/#ÚÀ<¢Û2Ál@|1~Ó?ÿþí+%Â?¿€®¼šq?­rp#ÃBy?ñ¨—³æKú@…žß(Äð¿êº ¸\R¿Á+m—C¿äOc 8o2¿Û¢"#揿×è÷»7ùì¿ëëgÝ^ëHAGNbll3FGL J0529.2-59171RXS J052846.9-592000?ï‹4y ˜
?ƒ6‡ÒOï?Q훉Ç;¹?HdQpè–?Šõ.&¡?'I²¹¸ÿ?ï€D#ä–?}uN†…A?7XÊퟕ?SØoã¡×?%hŸ™Ýß?ŽŒ¬Ï4—¨?î"'Õä?Š'ƹKJá?q«öbS[÷?`"Š×äO?¥Ò?«ˆ60?ˆ–ëÂ,þÕ?ï`§ì,+v?w°§!¾»;?^/]6Þ?M,^9µ×?'´§#U?vîGñ&‰‡4FGL J0529.1-0101¿ïût{/©ÄÀ2¸Å¸ÜUÀ:'ËÌòŒzÀ<#WóÝ@åü¤«Æm@'Èš8%
?Ýhüopü?Û*à~Zxò@0…ÔÀ·?ù|*­þ€y¿Ýpõ³ ?ïzËx8ö¿ç§¬_nû¿ë+$Á€hp¿Âðvà‡Û¿ï|þyØAGNbcuPMN J0529-0058?éc­!ʙò?Á_(¹ìW?º}¹hÞ®¨?»ÑôÈO½'?ºd݈́È?µ¯£v8?çö{®[?ɶ(€MÖé?Ãb×8ÏyG?Åh&??À‰NØw=?·ZMµ%'?æL"þ7vä?¬àœ'6G?¸¨`3]Š?ŸÜÃÜÇþ]?Êy»Àˆu¬?¦vŸÂF?ÞǚS«åe?»<`u`º¢?¿hÁ>q¦?¸ M¿ý?Ùq‹|~1?À-ê'âӈ4FGL J0529.1+0935?ïYÎìØÀ*Ú ¼8*À:&ä›ök,À<[}Ë@ C~Öʧ"@†‹ýϤ?¼x‹×åп…aC^EýÞ?Ëxëä•{@gmrU?á5žÎ^¿Ú>(¤äÑP¿èQxbè,¥¿á8Ï>ìúÀ¿Î/~Ȳ῿áå]‡š"•AGNbcu3FGL J0529.1+0933GB6 J0529+0934?ï*Î2N?F‰rß?`Ì
Y&?T'®"?˜«l¸q¥?•~U&}?ï…P"´©q?Àîê'
?:Óv±ó
R?MŠäBî?ÕCFZ?Žªî*z-?ìp
E*ÌV?¡êª*žª?…IM´ð…?u]þ
;g?¹Ör,òÿ@? ±†	ɗ?íÈRïó?:ªi»"?kÞô°\o?^RõåÇ?°Þ~ˆâ=‹?\Ýƈ74FGL J0529.3-7243?Þ'XúºhÀ?à.D¶é6À:YDéN
À<Q+"€ä@mÑ Ç
k@™µc#»Ç?À*ZÜð[r?±:ÂÇ;=?ñ4+
oÆ@4"Y8«m?ÛL»ð[¿×cL@Í¿èd^y]¿Ý"Âãü¿è˧¾uq¿äm´8PÍAGNbcu3FGL J0529.8-7242PKS 0530-727?ï¯Õ-.ÃD?ŠÍďNY'?[æ®&èüe?k"²ß%?€ÞïrÜ?"…Bº²ê?ï¼÷iŠ?€ùÞ¡Ò:°?.°§ÈyI?D…¤.àT?€G|	2\'?€`Ä¥PQ;?ïßߞê¨?"À'ñF?p5ÆP†0?eÎ…©f¥?›6'x'?'¸ÂËd`?ﲏ-"û?f¶
h·ß?P3oÂË?8­ÈÙÊu$?UÈü¯?fc†i,­´4FGL J0529.4-0521?âÀ;vp5À4§"BAÃðÀ:	"V!uÀ;Údµ—&@'»Ÿ}ß)@E&z¾@?Èi
!A?Ñøá}³à@)=Ùb·@´Ž®¯?ÈqȨü¿ä®Á~ºñ¿ço£üÉë¿ë#3 hÖ-¿åù)Í¿ïîäŸQiAGNfsrqPMN J0529-0519?é´Ý²Á¾?»ê¬'ª!?¨ÆóZG÷? ÚüëQU?ÂúÎÒ£1	?¸"á~8ÂÀ?ë; çc=}?¹¹Êð,x?«¥µ.Lœ?±àòÄì?¸T:NíÉ?¯¸ö¸Çí?å<L†¬?­…"Ãà?´ÛBXV/ž?–ŽPñŽ1h?ÐQÑËfÁ?¨ÃêlŽ<?䛒*R|?¦–°"×lø?µ˜´¬€k9?˜—›¡:º?Ñb®€Ñ@9?¨'â¢m§4FGL J0530.9+1332¿îÊ`UL°À&YWŠ*'À8Œ×òš½À;={á!îg@%C"d(I@­
?#?­êYXR…?ÑÅ9$ä»×@¤
COàé@0à?ÊN½þ'㟿Ûé
_¹ùá¿èVݲME¿é55¬E¿íàpÀ¿Ý,_#ÑìFAGNFSRQ3FGL J0530.8+1330PKS 0528+134?æÇÜ|®)?Ãô+²\uš?Ï-Œ$ož`?ÂS!£l<?¦Ì
Æv£ë?°¬/+%ì?îUÝ\xë?¶·u½…œ?‰ä³™®|?¦Ð"Ždޓ?¤)sÌÒ?°^©»uÌÝ?á–ÖëøbÒ?³²KŽ*±?Ô9]Æy~?°š,eÅr?Á1èā¿?¨—ΐi'?ëf÷-ãB?¨Jg/××?›bKgy¤?»ž}+'?½ï£>	§‹?¥ð¹¶ÿ34FGL J0532.0-4827¿ë)H3~XÀ@fýüÁrÀ8;u!MÀ;g¤(hÔÖ@]
È°ÞZ@±ƒ›*"R?žTþ£Î?­?³è'¦
k>@c5X§a@ 
2~,€¼¿Ðëæ£7¨
¿Û@.Ä8©•¿âËcÁ'ý¿â[Kµà÷ý¿å6±'n"ÿê^òԞAGNBLL3FGL J0532.0-4827PMN J0531-4827?ï•òž2F?}QÀ.P7-?=vÒ=á6?4ýn­£:?‰—¡á‹äÑ?|ëðªm?ïÏXìë*¯?zr<?²7£?0ö!èv>?Kí$²Ìl}?wD'kã?Ø?y¢¤ýx:u?ïê~?5¿®ŒÖ?~yҝˆ·?|Ñ$Ãâ,?˜>î®7s?‰kAùHî˜?ïø˜ç?ó?A™zøð>ö¢£ï7±>ö1î»=ä'?Nô‡Fx¶÷?A{O'¥Ñ4FGL J0532.6+0732¿ÞQ_½À+uîÇÉXÀ7"ñÓ'éÀ;B™Øƒº4@äÄ*;è¹@ž{€©ß?—w¾8Ɓ??¸
Xs‰@-š
^ÿ@kß/ûÆ5¿Âç<9¿áyÛX€Ê–¿åô>‹$¿äN'ÿú ÿéÂ}h‹…¿í*7/AGNFSRQ3FGL J0532.7+0732OG 050?ïMõòþGŠ?ŽÐsσ[|?ef
ßô'ì?eœ'À¡hT?""ä8|?Œ!á¿`%?ï"=ϑÄO?– –}?]Õ£¥l#°?vˆÜy.,?‹5צáh'?•'T'_!?ïRJ;ƒÕ?"Öi;y?{hQk»‰›?wϛ›ñŒÃ?¹Hi,õ–?~;f¿†åÒ?ïU'Åïo»?ìYÈ42R?l\Ü΁x?^ûIgM?'Â#Æx8X?}3Ÿ‹ðw4FGL J0532.8-3941?îî4/ÝÀ?p‡¨ÖMÀ9¦Àð¸,À<]sWN›@¯B¼I@hÀ³¹Ö?°°"Üj ?¢ÊîË	K?ì•Õ>á<F@
£	Õk׿¿ß^TùM¿äÀVìÔª¿è¡Ü>ñ§¿èáyaë­c¿ßúþÄÄ
¿æïËoÌÂAGNbcu3FGL J0533.0-3939PKS 0531-397?ïëÆܼF<?a"Á™ú?,ž±5N°?%â`Zå±g?boB¸¦pr?`Z>¿:ïJ?ïŁã-ñ?€6¦¹>º?*(9ü¢w?>Rýí×±,?|m̙"oG?–ì'å(?ï@ÑÉAé8?}tµÃ¢Ë&?eÃG¶?Qáu¦å¤'?•E®nÑ"3?{ñ%Mõ"|?ïéâSžHõ?Q'aÍæ*&?DÁ4!N(?7'åiLU?`íeÔ®·Í?NÉ[ÁÍ4FGL J0532.9-8325?ë"oIu%,À='xÝao‡À:ž‹¦'Ï¡À<Z›•\W@ ceù"ð@$á{°z‡?ĨèÁõÙ6?½š¸}ŠoZ?øNbS—@·ww°»Ÿ¿Ù‰§^(T]¿çv•žoû¿äêÖù¿ß ¾Q	¿ã~ÛþZ¿âÿ90£6AGNfsrq3FGL J0533.6-8323PKS 0541-834?ïä
¢Öf?6ÆqjÈ?$ÍêH)_$?94Š¾9q?j¸§î?€NÿÿÕm?ïÇÚtÞu?~Éuþ88?)O¹ÆAç?G5.Õµ¸F?{¯"÷^¶O?}dí{P‰?îð3É	O^?‡b²%ÀÓÊ?`s{®Ö?NÏQÄâµ?Ÿë{ P?†'bM"Ù?ïŽÉÏ4f?w|;]µÈ­?6ëá€Ã-ê?*»Wc׿?‹–-&øM?w'ž¼xtY4FGL J0533.0-8446¿Û'Ð+ځõÀ<Ädf±åÁÀ;g
ÑZÀ<…ÚcŽDÒ@ùX¾2*J@œÈ='?É<;±î?­Ø°A ?Þb§Êà@ÅÌ8þ#\¿ÊEŸœh?À÷ö†¯‡¿ã{Âîýy=¿ègÍ<^¿ÒÞI¡ßŽE¿ïõ£ñpwAGNbcuPMN J0532-8447?櫓mùˆw?|Bø0}Î?>1Zó¬¾?;$hót"?…âª'?{bdæêr?ï­D SQ²?…l&~žŒ?*A«ÐÙ¢ð?Ctÿí,¸ç?"EÑ;è-O?"ì,FÝ°?î YÓßSR?ŠciQÍ/œ?lr¾††Dƒ?b—ÅÆó4"?¤36Ù¢f‰?‰;%NU`?ïŽ^S|˜?rå:q3ׇ?5Í° ï^(?-9¦‰I?‹¹ýŸÒ}D?ré/4FGL J0533.1-6119?ï†<%†]ŽÀ@s(bõ˜žÀ:¨`"†ÉÀ<bûáN2@õÉe²@à´Zåÿ¤?Ì&ñ[wu?Çö?¨·o?ó	7KƧð?ïücÍÒ'Í¿ÕÙ6ýîü¿êBjۖ"¿ìÂ¥â'Qþ¿æ_Ë‹«D¿ïúè3Z `¿çb¿è¸¼AGNbcuMRC 0534-613A?ïѵ8"·?ƒJr²Ï?lÄøì¯Á?z'ÏA¥Œœ?bQÚ¨šÒ?z[~èn›é?é+Ë[ñF?Æ 
~ó?´/7ËK9?¾ÍÕ'†U?Á96®Z•M?¶Ì~ÓÀ?쀀ÊÂ[?nÅÀ0?™O4#â|?‹ÚÂqŠüÅ?µ¨, ô§?—¦8¢­Ø'?êeá:ºÕ?±Gx‹)°X?»»•µv£|?®pdžT¡?±`z+…Û?ìA¾øz4FGL J0533.3-5549?ïÛzBÍk>À@}Š2ôIÀ:')óÀ<rfàß©H@ý܌ˆd@£!ØG?вLBù¤Ç?ÕRåB˜?ÿ0ÈÚÏÄÏ@rßÆ?é¼|±¯¿æ_(뱔¿è'm{-ž¿ìâô÷ŽAw¿æ©Q2!»<¿ïÿ°NçÄ AGNbcuPMN J0533-5549?ïUlPEN+?"ðºö¡—™?smn¡†?r…<iœ<Ç?w5[­óÇ?'(Åu£?ìǤš:Òh?´D‡ñV?l¹)?–¹ô릝ì?µß÷­{Õ ?±ðMÓe^T?ë]Ez4Õ.?£q¸‡ÅÀ?¥ÖjH,k¶?'.œö9_Ï?º*Ÿ
C ®?FAm‰H?ìì.ð©ƒ?•B_(."¯?™Ÿ"1ÑÌ?ƒßÓܹ;?²6£ns/w?"ÁA]$)4FGL J0533.3+4823?×Vršs«–@ {z_A®÷À8t7	‰À;ˆ"/•ð@ï-Ì­B@–n^'lV?T뱤í?¶./g5Ä@øDIÛì@Ðw€üj¿¢ÞAbd¾¿á›CRe'¢¿åÉ(½äQ¤¿å¿˜f"²Ð¿è§ÂòXw¿ëô—ìñ/ƒAGNfsrq3FGL J0533.2+4822TXS 0529+483?íÐ,éõõ?£Úh€·A?d²Õ~Ôy?aÓæywˆš?°Ù1¤`Ó?£~¢$e"#?î·+ÿÝ?¯e9Kzn?o¶ad#4?ˆ'ì?•k:?¢'èQ½Ð&?®]P£wñÍ?îët5Ÿ+?Î´+Ä(?}³1%?w<úxÒ_7?›MÌۙ™?ˆ@Ç!«6?ï…{‰vã?sø–ÑTïÞ?qO)_ê•?`pÿ´LÉ@?…ùˆòC
?pœ^4»¥¥4FGL J0533.8-3749¿æo¾*üÀ>ÜÊ>}QÀ:¬6ÉÀ¨ÒÀ<šq
"=@ba§ºÄ@m(<_+à?ÅôšÇ)?ÃCOàèã"?çÐ*_z@ ›'
`?ïôb¦h_¿èuüÜ_¿ßéÔ¯ð4¿ëƒB‹?å¿åÇ-†K<¿'üyº´¥AGNfsrq3FGL J0533.8-3754PKS 0532-378?î÷ŽŽž?º&£y P?'a';b?º/Føú?‹Í"lÖ?Žwjqt?ï:‰ó"´?•éâ
U€?QðqÔɟ'?eЉ«¾?—ºqύ?"b5EË0‡?îRáÛ)?Œþ°ñ|™f?s××mxW¶?mIJEN»Ÿ?¤Öôžci?Š¬Ñ2öë3?dÀ.?t%udë½?TlÑè^R"?BñÙ?r?ŒCŒ½Ä)ë?sÔMãJ¾4FGL J0536.0-2754?é£îCøÈÀ;ÝCá`xÀ:ß9á£À<]HœQÿ@·FŽ"½"@Õ¶€Z-?Ëîc cbP?©sŠd§?ÖÏþ…Š@–ˆ¼|ž?î10Ÿ//ÿ箅^¤%9¿æÓZ»7y¿å·Š`@²x¿â¼(Fp'¿ïÿËA²Q÷AGNbcu3FGL J0535.6-2749PMN J0535-2751?ï\˜Xmx?æ´Àm?Uj],µ:d?J±×˜`^Z?"H"&ýW?œ+7ði?ïF]˾?'jÁ1}?LŸzÉ 2V?aøm€9Á?–OJÈц˜?¹Î¡¹K?íëòÖT4,?'[‹¦¯Â?ztS	¸×?kÇÐñds-?­òH9…»²?×y
·3å?ïZUÛD?{±ÎÜa6ù?^ºÊ'ÆèD?Kec¯2 O?š)œqÉ?{BD·ÿ#4FGL J0536.2+1733?ïÞ´D&ßÀ5çB™Ø"À:Fêóÿ@½À<eO1Ì@}4‰¢?þFÙóü¼?¢4GÛ5ñ?Οÿº4ï¡@ÃÔ»®—X@Jæº3Âû¿ïþR`Ÿýâ?ïýýu‹r¿ÏëŽÄS‡¿á9‹Â@Ð¿ä,õÌ W#¿ëþ? ÿ¿hAGNbllTXS 0533+175?ì~Ê¡ Æ<?³:èüý½?'ÌJN‹KA?ŒÌcPõñ×?·V˜_VûT?±_1
?éPÌèkÍ?ÅBc"W˜ð?s¥S]6?'D< ±±š?Éaç¡Ãd¿?Ä÷­½ÌQ¨?èS}0Bk?«Á'w°?©"ƒà"…þ?•mZ(Ȩ?ÈPêFҐØ?¦5÷ìÈm?ëäø"$‰µ?›¡
n*?–	ݱ·MÏ?'Aó¤\?»UÄrmÞð?™Gƒ
\¸õ4FGL J0536.4-3401?ïL›G!ZKÀ=}Š2ôIÀ8¡è
šó6À;Ý6'Ú9@©½H@û0<Þ­ ?¦'a;Ú È?µ'ƒ§"Ùì@í'ÞkZÂ@/cê¶Ó¿Ø6µž²Þ¿âÏi)Eƒ¿éY£àDxÖ¿æÖ_îÉ¿ïCB	[¿ïÿ²vìAGNfsrqPKS 0534-340?ïõÂýDƒ
?I"hi~ÈÄ?@º·§†?88cYæ¡?HäPß<#ü?Cq'F³"î?ïÁÚf4jž?ƒµ©Ó?3¹ÜK«M?H}K"–?}×/!ûË?'lä<@Ît?îúS=ä{©?‰ý"ã ?€~ñÃîë?yMÆ>?˜vPJŽ"v?"r7+?ïú¤(ÇË ?5åô[?!nW íÛ?Ê2ª8Ák?AÚÊéG«?3u2¯÷…4FGL J0536.4-3343?ëŒüÀãèüÀ=h"ƒ‡ß]À9L&ÉÀ;ÏÏò=@!‡	^Ú+?ú|Y¸:m?´âlFOD·?»rØ Ñ­m@
pÇZ@©U¯	¿ÙZÿ**¿¿è֞b+CP¿Ñ'd@ò8—¿ÛúcWh¿×?d"cýV¿Ð"c:AGNbll1RXS J053629.4-334302?ï‰7O?‡g:èÒ?PXô.ñ\ß?H©"~+÷3?‹§wMð?†È–µÌþE?î´-¶;
?¨bepã¡?rÓó~"ï?*î7]+?¢b¦;?^˜?£=2Ïb?íu'ñ,
?¡<çBÚ?qo|<ǯ?ið@eà¿ç?³<ð²Þ'»?¡]"í¡?éWß«BI%?§ëc7'—€?"K«R¶zu?v:Aà²?É[ƝËsÃ?§ßP2T¤4FGL J0536.5-2548¿îØi ˆ"À;Á?ÐÐhÀ:òÚ¬‰`fÀ<¦"Òb8@ 8»*
Ä?ûî[ãU¥N?Ç.DáÜS?Ãí†*Ñæ?üÉåvç½ê?üku.€F¿ìðdaS'?ïâèÍ´SY?É.Êî¦;i¿â5Z 	 =¿ÛrMºÈé=¿ÝïN¢$'–AGNbcuGALEXASC J053626.90-254747.9?ïfõ/S?ŠD$ˆÅt?Vö²š†0?RMbæ®Äó?'¼ðà ml?‰µ"S¤÷?îÁ¦Ê-«?¡ 9;?eBŒ‹t6D?wÉG»sg?¢'ÌÊ¥â?ŸvP
^?î‹I©Xø?A¥vǁ?w¾ºç‡Ì?hÝ4Ò	‰;?¬ty3?þDEÈ®?í%8¤Äї?—­©xq›¢?¹S ãÚ?v'À`¡?´ŸeVÊ?–Qy®f۟4FGL J0537.7-5717¿µ½5þÈ%&À@2'!%¶À:/Pž~éÀ<}`Z³«@ñ:ǧ?ý~"_¦XÅ?ÁÁ¹my?ÆBº$Sœ_@w´_½Œ@j/š¢X/?ïÉ­}ÒÝ¿æÙäãD¿Õë&>®Ÿ¿ÜèÿI Û¿ãèZ&½+¿æDiò!vAGNbll3FGL J0537.4-57171RXS J053749.3-571844?îüÌæ'?' hÔ¯+\?w'ûŒ€ÄÂ?o ,ô×ÙÑ?šäYmÜÇ?ŽøNl—•#?î\œ©Æµ?©3M"ûÕ?uϹw4ù?€–È-fõ¦?¬€?®
?¦È¾Lè›é?ío¼R§H'?–f·Óe?‡âDø¼r?{=æ©Í/?±…ÔË®+¶?"
å¥ü~-?ìÚf©q?œÚ9Œ¬Ã?'a48ï?u{b‡?´×¹½¦<?ÍJéÐ3Ì4FGL J0538.2-3910?êN€e.ò¡À>LøŠ/À:îäŸQiÀ<­C³³÷@ ͪÃ7£?þS#ä
Öô?ÄUaÆÄu?±ÞfRDp?îªõÂ9uí@}
yæ ¿î˜×'2tÇ?ïömzVÞ3¿Ø70£‹àÉ¿Ý;êý9|#¿ã2½ÂmοÜl+Â{AGNbll3FGL J0538.4-3909NVSS J053810-390844?ï÷âÞàý?Fì)c/û?? å¨xZÄ?Ÿ]|@†?LÀkmÐ?ERÁˆ{Šã?ïȍÆH`5?#ÀÒÓ?'³e`<?A™ôÞÅ?zû°ÎÚ?~H*œ°d?ï,&5šß?{ä>òä¦	?aÁÒန¾?P%ayA?˜C}'˜?zgÉýü^~?ïÎć£é?^¬TÄ×›?@ǂ~¾›4?3bíâ?v…ìV7þ?]›ŽÖò4FGL J0538.6+0443?âì^Ÿ¿ð¾À+³ý">5ÆÀ;]{ÜqÀ<g$€	@!Ã%	òó?ò«^Öw?âvÞñ'?ãÓÓÃt^@ÆQÒZ«@"6ÙÁ¿îè"1 ‹ü¿âݜ'éS¿ä5åàD"ð?â¼(+ì¿ØÖ'\ä¿àJÂ7óaAGNbcuNVSS J053847+044222?î?5ÏQV?¥PÖG¤v?áî'É?~¨ÀQ®1?¨eNš'z?£¥:üö•?í¼¼_>s?¿Oі?p«{ðŠqò?™u$i>a™?±hýeU?¾>탿?ë4—mÂç?§ÿÁ¦0–?"Î"ËÓQ¤?ƒjH鍖?À³ßxΊ*?¦³¡ÓÆ?ì.*™ôçí?©n)ߣ"Ü?YYÊÉÏvß?l¾íØB¨2?¾)D1'Á?©S[ñ‹8Î4FGL J0538.8-4405?Ԇ—N:˃À?"á¬WâÀ6…C>C1®À:áUÁÓt‡@¹&>{@%ن³U?…/‹]ìšH?¯¿!M@$qJG
@"_ða俚£xHCÄ.¿ÝUý£z´¿âŠ¨ÀSÓ¿ás¤r:¯ÿ¿å~bÁ–7å¿æHdÞ&‹AGNBLL3FGL J0538.8-4405PKS 0537-441?ïO ¯âK?‹LŠ>˜ÿ?P€U½±G?Ql9»«»?•ä§ãâP?Š|›=l»O?ïxx¥&?™Géð43?L­÷ué‰'?i¾Ã!ge?O«ñ_?˜Ò1šÔQ_?î"¡'¾µ?™CJeçVï?‡—µë±ô?†TIu'0? èÈrÁè]?"é+ú¸¨¤?ïõòž;W?Nã#҄?
b)ÈDôK?+ÒC"?SGc5G*ï?N7)–4FGL J0539.0+1644?ÛZ­ÚˆÀ²ðZpŽÞÀ:?LÔÄèÓÀ<ƒræ§i@ À-+1\?üF€'q^è?ÇÄÚº÷f?Ð#nå;µ@`q$/Š1@Rëä?/@¿ïÿüñý?ïý~›;…¿ÜkÊSuÈÚ¿Å÷÷ÛÉ¿áL«tp–¿ìÓ51:4¯AGNbcu3FGL J0538.9+1646NVSS J053855+164612?ìçÊàÜ?³•Ïò?qÁˆ†?fÑVã¢?¾$±_hx?³KÆuÁy?ë@Ãd3¯?À–i|IV?[6
Ò§æ9?oB¬YÚP™?ÂƆY‹óæ?À|†·ï£?é4yj¦[ñ?­!<¿?žüºï:'–?@j"Ö¯?ÇN'÷KH?¨ãö»"tÈ?í/ÁSí¡?'š¾1ُ%?…'h™
tB?rU"ÚÇ&?³ÝMq¨ì?' !†Ë4FGL J0539.6+1432¿ïûôGm°À!_ôºQ À93Ô¶¦ÛÀ;©žÙt{@ó+kh®À@}/Bãª_?¹LFT£w?Ågù¹iï@§î%âè˜@çZ™B?ïø¬N¨À¿Ýã܉Ù2¿ç1Ubˆ
{¿æ'òÁS¿î™i}Èâ¿á€‡—ůAGNFSRQ3FGL J0539.8+1434TXS 0536+145?îÌՀºc? ˆÔ^ÉÛï?vZåäYJ¹?wå`‡]? gK7Ԑ"?‰ö¡5Òo?îFû2'Ž?±¡×ßm?Fo_ú£?_ ý®Ê«-?«EâGVüƒ?°ñÊ7¿éÌ?íˆŽ@?™í¾ˆlÈ?''³YIz?Žã7°é?²ÏRÑIJÛ?–	:Âñ?ïI¥_är?{ñ •Ð?e¡ƒ&Œ+Ý?SKùî­èð?".¯1ì_?y"<·Ý'î4FGL J0539.7-0521c¿á÷œ¶w¤À2_5ŸôýmÀ9ə~Á¦ÿÀ;T²ò03¤@¶FÉ)@0Þ@'—?ÑáõRýÔ?äŽàØóL@-d"¿G©?û½DC¦É¿â†¤^ïy ¿ÑYƒÿÔa¿çãW=SŒ¿îýÄupÅ¿ïþï~þbÇ?ïýß(ïãRAGNbcu3FGL J0539.2-0536TXS 0537-0524?àҊV}Ì?ÊNåÐ*«?Í$Ìý^?Älªms?ϑ
½¤ït?Ä$ì'Úå¦?ØG©HŠ'?Ò¥ð‰?Ý{=ùô*g?Ó\ËF9£»?Äz1{‰)?ÀkújM?Ó0ↂ=÷?°Hj>¼ÒU?Σ‡Õxëm?¬ÜQ™¨>?Ý}YŽÁLS?±tf²ˆ?¤(îkÓÝ?²Mâš?ÕIè?·x<¥ÅI?äí"ýÎt?·ˆ[œ†ZZ4FGL J0539.9-2839?쫦ÕÑÀ;FE^®âÀ8ÜhìR¤À<:kHM@æo¨"µ@jnü7£?¤àš_]u?¼£çü(/@IŽ|/%‡@³puÞÔa¿ÒԽ렿æV¡ÍD¿é®/RÓâk¿êýDcÝ*¿éÒ%Âu:¿ïÿùëñAGNfsrq3FGL J0540.0-2837PKS 0537-286?ï÷Ø3غ?GêyÁ_ü?6ý
0:Žô?5*ÊRáÁ?E ªú ±?BÁ«¡Áp?ïzÓ‹}F?èktì?bwœ@éyk?'+G0—‰S?Œ­WLæOÞ?¬ô­Þv?îêwâ8E?ª!0ܯ?zU½Â0Y?||ÝãG&°?œ¯³,òß?‹ÚÇ7¶?ïÀx›[?luþoüçx?o"GÆ?c%³Âüó'?p<ãŸéîX?_R]¦Ø…½4FGL J0540.0+1209?àã']ëÀ#©QçS`ÐÀ:MY0ó½ÒÀ<ږ¹ëI@1tÅyÇA@b‹°¢Ê›?ÁÅ«âqz?¦í´£á8?ç*êßÝJÉ?ÿêEko׿ß;ž¼™#¿àÇ÷°¦%™¿è""j«o…¿åÂù¿ŸԿՏF¹!õ¿ì©«àn[AGNbcu3FGL J0540.0+1208NVSS J054005+120955?ܞv¿c·³?Å8búžƒ®?÷õ¼‡T?È=ßÄ&ý?á0äÉ\µ?ÅN©9þ¥?ç-rxJûa?Çûu®eçÏ?e[žf	¿?tÿ	æ7Ÿ?Ñzcҝ÷?ÇӒ‰#þ?çë‰$Lœà?¬ßr‹?œZuÕl›?'%a÷®cK?ÌÑÐ Þç?ª"¬k`?ë*)>?Ÿ¬¿}*Ǐ?ƒ6ü>'æú?sä`d¦ö±?ÂÀ_"rT˜?Ÿ‰ôGS(Ë4FGL J0540.5+5823¿ïÿ䞝@,‡îõìÀ9·É°¸šÀ<1µ°P•D@ {Md·»?ÿ4ùÜÐP?° ÄÍ¿ƒäª
I…?×^ëîù@ê6êø²?ïªÏL¿µTÂ$'Q©¿æyWÊÆb¿Öt{/PP¿â*@Õ³P¿Á6"f\UkAGNbll3FGL J0540.4+5823GB6 J0540+5823?îÃސÜpÍ? êè÷¡Ù?Z+¦pŠ?WŸUZҏ—?¢ñu•nÙ? ŠWßWß²?M+?¡žÇýºlœ?ZµbîNÍ?j: \`%?šÜ1u¹?¡*K€U š?í±Ï3Ø¢F?—aU-3Ë?|	(Tñ?søþy¬cb?°°óßÕ¬C?•ëµgÖG?íoÿ›g£ƒ?"¯Â!ÜÂ[?'³ðþÜ?wÌ¢ê¡Õ?°9Öc†¤+?'Nɱ§[4FGL J0540.8-5415¿ÕZA"öÀ?ڄœ²RÎÀ9Ö­'¿À<0'5G	ª@P®äY†Y@×¢~D©}?·…ß'˜J?¶vÙ{0øÆ?ù¸ÞÙ>Ë@üwÒÊgÃ?éÕá[Ð
¿àÚçœr<¿éW°´hR¿é
Öøj
¿é–š«èP·¿Ó3«¾Š>ÞAGNfsrq3FGL J0540.5-5416PKS 0539-543?ïÝÏ~¦ÿˆ?kšŠÈê?B0
wãÕ?<Rÿ4Ú·ë?m¤~»'ó?j:õ6ô"E?ïÀ½MÏÁ@?}ê5™c~=?,Í$vqː?BXÖcÿí`?~ºïôkÑ»?|þªY¿/?ïR²j´?'ÔŒéؑ?o)¦·yšÕ?a‹_¯5w?štÛºL?€šô¯ó»Æ?ïÕ÷Ô΢Ò?]Ó­}ËÍ?HƜ¦²í"?6Šû$Ä>?qëBØ:c?\4‰£Í34FGL J0541.1-4854¿Ó1Ō‰HÀ?[ÂôÀ;Jh˜À<»ú`ƒÎV@ I'ˆ°é?þláłU°?ʧ6eAÎ?±ç0Ñ.0j?æ£ø'Ä@Áp¾0a?ïà¿ÞQÚh¿ã8 7­ì7¿×@-…öú¿æûm"X9? ýÜåÑw¿éÝ}‰˜š–AGNbcu1RXS J054106.1-485408?ï'¬°øP?"€²uœn?Kº–Ÿ³È?Rßa^'?š-|*ËøŒ?"L_Ô#?ï5â\‡?–
PWŠ?Möm(GY?aþö$"?˜TÄtŒí?•67^wú?í›Ö¹­§^?–+"uÉÅÄ?tA˜áü ?häF;d¢?±Ý0¨´¥D?•pTm#'V?ï-Ìn‰)?†n4#7?D¦ö…ãY?@ª~À—ê¢?žU½ÿÀ
?†
¢o4FGL J0541.4-7334¿Ó‡±w†ÊÀ>Þy!°À:Îނö À<qÏI~Ï@D>·Ë³È@o?¾[ðÂ?ÇÍ|µˆ7œ?´e8>ŠÕ?ìÌxžÍ5'@¹\Øs?îñÓ'é|¿æPµà!=g¿åt!N¿ã%€Uпæ¢'Õ¿ï÷z?·%AGNbcuPKS 0542-735?6à=?•§ó¨ÂÔµ?d06J
£x?VsxÉq?£'k§ñ"
?•PÈ;&Y?î{ÚŞ
?¢äµüål#?eyŠÈFú"?q‹$"{«?¦êÆG!¯?¡ÿWçJý?íó##?'…@ôCr?}$)«ì  ?gô_Ž	`?­*Hš©½?åW€q¯?íF	`Øt(?áJï h?'I'F™X‡?i"ö-Âf?³†'°i3²?Úi'GÇ4FGL J0541.6-0541¿íÍò¨mÀ2üÞãOÆÀ9®Äjþ{œÀ;]±÷^pÏ@,¤ÅFƎ@ÙEnŸ?ȪÚ3½œ®?Æ6·L2º@	zÓõ@S¬–¡l¢?ïþVèD!˜¿à.ñàW™¿è:#aÔÜ¿êsp-…¿ïçæcvÇÝ¿íyº×AGNfsrq1FGL J0540.9-0547PKS 0539-057?í…þWï¬å?°
<ó†Fô?…ý}‹Ù?†²¶ÍÆ,?±[PÑ8¥?­jØþׅ?çî%`¢?Ço7Mëî?ÀÙ²Ì°"?ÂÅ,«k3T?¿m /aŽL?·ݕ{®e?â´4à,Ö?³'L@7Û?°J5³(Ô?"†8
 r#?֏ñÒÜ ?±8YÞxÒ?ÊèÌé2}?¥Ê¿\—­?Á=¯¯"?®IQ¯®4??äe}ŒÒZ?´Ç ¨*"4FGL J0542.4+3547c¿àµx{æ"@ÔÏr™À9{ÿL{ٕÀ;/(«ôž@ý~®Ü¡×@cwá¸í?É©½(?^?lj£Aãû@gÀôQv?ø?	ˆ??ïÿÝ/ñ_S¿½èplN²Á¿é}ž¼C¿çQ˜Wz:¿èªŒ€¬bÊ¿ïý¸È3
AGNbcuNVSS J054218+3541490?Ð4¿y8«?ÀzTãœx?ž>÷½ö?ž%:H}?æþt°…sù?ÁUÔqÞ@?ÎbÝNáJú?Ç[>[0?¶¸f«?¿©ÿTlü?㹚'œåÁ?Ë{†	SÕq?Ôë0ÒF?­ê³dI/?¸¯n)Âäá?—bJp4¬u?ât‹"źA?®|+Wµø…?ÇI_Z9J?¦=7Á_i?À·2ºRsÉ?£M4
0S?æ ù"Ô»?±ˆ•ª*J4FGL J0542.8-3458?ÔâäசÌÀ<u?|ÌÀ;§W>«6zÀ<åÄ÷u³@ Ó,nÈà"?ý<ÙTšŒ?Ѷb'œOV?¶wÁ­‰æs?ènò&"©x?÷p'¢Ü8{?àÈ'Kžd¿ãÏi_?*¸¿·ýÌ^'Ýh¿àG>îRX'¿ÔÎÄɞ¿Ü œ'­ýAGNbcuPMN J0542-3500?îÖI´Ù?˜7Ì	ñ?E>ÊöôdÒ?@MÄËóYÚ?¢Fi†"u™?—Ú‹-Ö?îÓ­×ÓI?›ªÞlE?bEà…׍?r|c
ùáÆ?¡ Ä‡5[G?™6¬$Nr†?í¼â¾æ£¤?'ÑNàœèØ?q°µßÑ®³?d[¶rºÈ£?°ýÞªÍÇê?'c<ô;JŽ?ì±åËqì?™'ÕþhÚ?l͈KCý?b\Œ'8Åe?¹ŠjÏKփ?™šòÝ.¢4FGL J0542.9-0913?ïäèuÛàwÀ3^rÚ/­À8Óp]`-gÀ;*[rÏ*@¸	FOÆ@×üMÃØ?´ìÈÀ£ž«?ÄyÔttF@¥!Whœ¢@ãðŠD?îÛD)$¼¿Üø,AQ"¿é¡Þ¹q¦¿æ# ÄS¿êÚ÷½'E¿ï´~!nÑAGNbcu3FGL J0542.5-0907cPMN J0542-0913?ïuUèê™k?‰%€›HK?y`[*šÊ?v)ëí&ã?…úX0\u?'&g¥>Ld?î3«²Û0ù?­ù>Cá…ø?'ÎÊØY
%?£68ÈǬ?£Ýßf kn?¤`/qî|e?ëm±ôM&?§¹«±Pô?¥ôý%µKÏ?—ø´¢f"[?¹—ñ'°á?¢ÌłÓ'?æ
q2%Ê?¨#»0?ú?³ƒÐõ?˜.ÉÉ$öÆ?Î>yèNîO?¦$ÚLC¥4FGL J0543.9-5531?í°ø;C*«À?z]9–úƒÀ8´ŸVqüÀ; L?b@êˆü¾W?ú'åÂg=?¦ –R?±Íߢú@ìÿdύq@)øH¦Œò?ïÍϖ«¨¿¿Í­$Ù¿ÙW97Y2¡¿Ôh>Ã4G°¿Ûï?='—t¿Ùâöúó¦«AGNbll3FGL J0543.9-55311RXS J054357.3-553206?ïå>n7û?h¤…|†?6+:ϹÑ?8½O‡n6?gü*n"œ´?fNá©óŽ
?ï›%¬E…å?‹Gg#Â.??,¬Bj$?O>a|ÅC¤?ˆ=/Œ‹6²?ŠJ)({Fr?î՘ÄCPu?‹µƒ•N91?uJ‡¿iE?rö{žÇ¤?ŸúE‡» ?‰äÂ?îñs¡Bà?‡	t¤Î¿?`L€yk2?O$>¹Åú'?ŸÇû×>֐?†Â.úÒò4FGL J0545.0+0613c?¸âîë¦CÛÀ'qýiôÀ9ì0Ûj'À;¡[wN@ź+µe@ñèæ?ÎUlƒ‹æ(?âÕýÞâ@†I%ÿÃ@³ƒJLÕF?çÕ7Ÿ©~¿Êø›‡°c¿ê¤0ÌP¦¿ð?ð¿æbb™RLAGNbcuNVSS J054529+061955 ?æ`Ô o
ï?Ç\­'ë~?Æ`›µã?´²¼—`t?À}Ž´`?¾™´ë¨Ô?êÞ)q?Çñ©Pº?¦Ö±²÷€?¹<ÆàÅî¥?À®ï([?Ã¥ZÙ$?ÜÊ`slû?°Ó×zwŒ—?ÅuCf!'¨?©ï–~µsB?ØzýÙçѳ?®Ní0‡<g?èwÚ¹ˆÔ-?¾Q"@Þn5?"°}GÅcz?™ØÙS?˪…päÞ?½iò6ëg4FGL J0546.9-2206?ìg"þÀ7 E®_úÀ;~?SÒåìÀ<̍‰Àß@!
¯Û¥W¾?ý¥È–Ý&·?˸é?©"ô›ó»ú?⥡õ¿?ÿëWã俗…"úÙ®?ïùõß덂¿ç¿Àéz-¿Ö—
]¦ú*¿ã/5b7'£¿½ÿ¹3<îHAGNbll1RXS J054656.9-220500?ïÊ¿EŠ·?n{X"†¡o?=ÇíQnA§?7|RŠµ4?xÃ÷ˆ#À?mYßÃèÝ?ïh¨(_ˆ?ŽÆÇÑè'?F,ÄÝѝ‹?Wˆ9AAn#?'9"Öeá?öo#
-?îF@R£0?3çÚÈÒ?lЛÁÖ'?X€Hqå'?©Îñ¯x?‹ä€w€o?î=8¦_º?'ÕÑïÅM:?{JÇd¤¤?oq£ñ [?¨ºlA"_Ä?'®ÁSeå4FGL J0548.5-5218¿ãZèåÝÀ>‹¨çv°À;dÿÑÜ×À<àNú9¢@63Ÿi½3?þ^Õ®Þ]?ÓDE>Îqè?Ý\Šû>Ë@ØÌ<"Í@à\Õîßq¿ïÿ¾…{ª?ïâFj^?Çi^GG¿á'V½•!¿ë•ö¬š'^¿ïíFõ‡ÖùAGNbcuPMN J0548-5218?ï<uýQQ?—
mÝÕkð?}#ƪ^Ù?"#$Mɑ?'(N«DõV?N§
µ¦`?îhÐë˜Ý©?£ÀÔKöý?twÀðÞ$?€Ö+ƒéò$?¦ä.T	Ÿ?¡Cäe8×?뽿ª§©?¢uš|?§N&4Kò?'¸Á§šñ?¶jô—­¼¿?›§Fy‰~?íêŸi-?"*ÎêK6?5ñ-?~´äˆòá?©›8'#a»?w¡0—%4FGL J0549.0+3258c?á7Ý.V@Ä{'W]µÀ:e²ÑyøÀ<Ô€ö@ ύ3YÉ ?ÿ­*:f-\?ĚS¾C4?²þ½à ¿(?ïïãB/$†@‹99\˜?ìÏt…
?í÷y´!]?¨]‰a×Ð%¿ãµÁM<ɵ¿ßЍ]b²¿Þ•Á}ŽK2AGNbcuGB6 J0549+3258 ?₈Õà¿_?¯Q"nÐò?‡ÖAsh?€a7´Oy"?Ú<<G¾U§?ÂϝUÔn?ä8qs<¶¯?Ê¹§"‰?u	Ô_P?ˆí?UûÇ.?×;ò6%?É¿"/ú¯?çaþyÈJ?¨ØÕßY™ë?–ÏuO»†?}tϲÑÎm?Ϟnè†?§7áþ?ê´ìuWðC?¤¡ŸZ©Ë?–Íð˜Zsü?Š~Ê8Ìo ?ÂR"ðs?£†5ć]a4FGL J0550.3-5733¿ÜV y®ºÀ>´üvÄÀ;‡‹z&À<§—…Ã#@@§c±«3@¸¤ÁëÈ;?Â{A–£E?}s±¸ç?»i"d O@3Yàqs?ï½|˜%¿Ý¤q"&À´¿ç>A¹Þ³¿äz/ ~û‰¿êBª¿±±=?ÛÒHÂf—dAGNfsrqPKS 0549-575?îòvÛ$¥?˜mʞkým?fÿÀ}å.?`úÂÓ?žÑ,˜û£0?—³´Xdjv?ï'*.Ž1I?šÞô?POr"—?]ÙP"ˆgä?šÃ
8>k?šT oý€?î+pDVt?ç»/7?záVÂ[»š?qAÍõ;J?©ò>#o!W?ýj£?ï Ý¸B`?}ø—èP?c94"š?Rc]vå¨%?™ë½"g ¿?}¥{…ÃY4FGL J0550.5-3216?ל´è:ÎÀ:.—á2µ_À:EÂHåL À<eg?ª9û@ 2x'$"?þÔóý">6?¶™÷']ῚÎL‡JÀ ?äØ<l—ØÏ@–ß~*R¿ÁaL ?¿â™baÉô€¿ãžë}'ü¿ÃøÄwhÂ6¿åø£_–¦¿È¢›[e¬AGNbll3FGL J0550.6-3217PKS 0548-322?ïh`ƒ Š?"7}úœ"	?WoÖý‡Í??L(öÝ—?'wÃqþ?ƒ:·c7é?ïo6vm?¦t¦åÌã?H2´iÝÓi?Yú"r°ß?']œCÛ?ŒY=+Dös?í¶yþN$?"‡Qh?zÛé<nßÉ?fÑX«ø?°žqyÇíˆ?"Û›£?î`8^
?‡I˜<÷?y¼¢þ†m?gÕMÈUY?¦Ç‹Š
Nd?…b²«ï^4FGL J0550.9+2552c?àZ&|ä¿â"Ùîô?À9æã3@Ÿ-À;\€¸!D@q`-…Ÿ?þ£Ah€?ÔVK¼J?ä±il«$@'Á¯bY?÷îÿ&¼,¿ítD
õ?í®¡žJÙB¿ÞГ@d8¿äì;\Í`q¿ïüá1ޟ]?ïzô}jäÐAGNbcuNVSS J055119+254909(?®Üx´"¬Æ?¦©­&ò‡?—Ãlí
|?›ÒxÉ
´u?íTˆLÆ?®UÙïƒhé?»úŒFáýÏ?ÀË{Õ÷Ót?¹î;°BC¥?½yˆ¼?éBçwÑ?ÄáËJ0?Ç3¢žøÁ?£éÂÎR:Ž?ȓ‰ý!?£OQø~?åŽ4ØùŠ?ªg©ª ?Ƀy9aÇ?²ð\
á±?½«ž>ë!m?±€ÁJ.,?åéÉÔCa?½¬ñ–3*4FGL J0551.0-1622?Á½ÊG<«À4ŽùÛ"ÐåÀ;jNÕP)
À=<±¥)@z8MNgl@‰üpy?Ôa):¶à&?ïü辚Úâ@n'"šV@Ÿêw­‹"¿ïè—8å?ïý2%9þ¿«s€]æï¿æIàô¡þ¿ì³·RDÌ¿ïÿæÀ
AGNbcuPMN J0550-1621?åØéÁ±Gì?ËR?̱O¦?Ò-®"<?Ê;c™/ÔÜ?¡–sÙ f? í·[bª?æqTïK ?θþë®Ý?É82ÏHT?ʽÿap|j?ºE'ç]?´[÷Ã4?á.±w-ð?´å\$Ê?Óù¯…"–Y?´ØÊDË?ÃQÛ'?¤¯"½Ì•ù?èŽ$¡Ýq?´uÕJk?É»"Î^?²y¯©‡'ä? 1WÑݶz?"fB'FÔ4FGL J0551.8-3517¿à~kÊö«:À:¿ÿ›V2<À;_ø[ÆÐÀ<®}1"Š@7ÐVD/Z@80êÄ?Éãã¿­€¿ªÕ!ș?àèøFΫ@û‰"Óê¿ÐÊaÛ<Q¿èsáÿcøο蘰C)J¿Ò·ÇíiûF¿áß& {±¿ïÿž´JAGNbcuPMN J0551-3515?ï±ë͎?|Àhp?S7²PH,¢?GP ÚÊ?WŽÂO—&?{š×m›¯?ïkT½£lu?Œp¡þÔ+??*qq ®p?M…˜k\?'¾…Íî?‹*œ¹1š?î?ºÜ$Ç?LS?ån?v죍&²?f…¶ªM3?©&½ÅXã]?Š¸A]ß؃?ïD`Ha‹?€'3Ã?Q…Ü{¦à¯?D†SR,å#?–[™,$€Ÿ?¦ñàÕJ4FGL J0552.4+3755¿ïHsò@#Ü@G¹EÅÀ9£4EHßÀ;º]éÀ"š@n¬`@¡59°€?Á—O Ò?Á2ZR½?üzžF§">?ÿÿa¨â¿Ðqm*¥Æ¿à)û|ÀÙ¿è¤@¼ˆ±ë¿åPŸ?J螱Áƒ˜{¿çWÿñ<nAGNbcuB3 0548+378B?ÜìÎ'ÚÊ?¾ÚßX«ÿè?´è©6ö?¬"j°ú"?Þ§èñ
g¸?ÀšXGUû?Ø[ÍÂØ}q?ÊF9†+ìµ?³«G‡;r?´¶•ÀVz?á\°-¬_¹?ÉDž5îy?â6ïýžÈx?®¦øœÔ¼÷?°†Md\L	?"©ÄŽ0Qk?×pŒ««\
?«È@ۂš‡?ãŽÏéƒ1?¬µðÔû ²?´ªóˆ¦Ã?"P}ã}"?Ó·£K­u­?ªÏÎmsÍ4FGL J0552.8+0313¿áÖÈõ¸åuÀ&ñÖ1riÀ9Øe8hýÀ;eQ‡²‰@q¡L–[¢@Fü"û­‹?Ç´°¶Áš?ÑàZ]āO@
ûÅ<@ÿ7VÙUœ¿×í\¤Æž_¿ß&H>2?ÿäÛâ…ï¿èòÁˆËëü¿å«hÎör¹¿ïþ3AGNbcuPKS 0550+032?ì;šé¼î?ºé0ìåÌA?†³û2¶"?4s}2›?»L¯º[Tç?·Í/ª÷tð?í9r_9)?¹pK|g/z?'Q'4'?¡Û˜ÊUÌ?³1êŸâñ/?¶?qhŸù?äˆÄÂ?±!"ìî¬:?«u.¤QJ?'¦Î¾®"?ÓÐ¥Žä\?¯rt˜eI?ã?†\ây(?¯y /å¿v?"5ЉáÂj?wµ´Ô#!?ØM–=œñŠ?¯HBUÒjã4FGL J0553.5-2034?ìÍ¿ª5¯KÀ5ž YžØÀ9Ýu&Ê;À<­ê‰v6@~¸w«?ü9 4¾M®?·
´ÉuÕ?Ã׎\Nµp@ÿW}•@¼E˜•?ïüÀO(\¿Úx6<Òï&¿Ñ°'#Ùy¿ÝóÎCoks¿áè–!?é¿å[Û]‰HAGNbll3FGL J0553.5-2036NVSS J055333-203417?ïoŋ*§á?¢œ`@>¬T?…EM4Ή?¢s%âò^?~¯ÐBr?t©wi'Ùu?ï±ö{?˜'ªÒ½?h'ú;‹0?sin¦x?›Ÿ¹Ì«Ô?•òã.‰¶	?înëoL¦?'W6ª±1µ?‰Ày#€YÃ?†)â#0Z›?¢¡0°+(?Š/þVß¿Ù?쥷ë|®t?˜Uúøó€‰?ˆ÷"£ðk?s¨
<—?·³P¹îV?–ÿ÷e¶4FGL J0554.3-1009c¿ß!q¦3[À1<yÄ<hÀ9ÖÁ['—À;¢˜¢ô@>ñŒõœ@W'"¬Ó2?Ì°rùòŸÅ?Òc¿m@ë_ïIÏ@☡!"e?ïû%|'¿ÞôÔRÓ«¿ç¸}õÏ$–¿í—'"Yœ)¿âùƒ¿g´o¿ïü`8NûçAGNbcuPMN J0555-1002!?èrç68E?ÃGæâà¬Î?"£Zez?Ž¹6´sÁ|?Ë¿÷ÚyÜ8?œ19IÑ?ìª[!˜F?´1¯xÁ?š:öÄh2Þ?£›ã?´iB%'?­vÓ,f?âb鈥 ?°u3Ãèˆ?¸Úé¦IH?›©†ÁÞ·?՞Ã\tm?­qSî ±ê?å×É$ÄÂ?±M'U¨›?›êaÙS­É?‡tÛ·;Ÿ?Ô;ªP!;ž?±?'¶4FGL J0555.1+0304¿ë
ÇÇæoFÀ&¬ÿ§ëlÀ9•'ußÀ;;\ºëù¹@"©	#?J@X$¹ó¬5?ÒXDЩ*?݀£(Ž"ƒ@kE®_ú<@Üƒ#5?ï½<Á§TÿÆ?¹éÆ,Ë¿êz73rô¿êm3t¡'Œ¿êõÀv}4ß¿Ò¶žb+CPAGNbcuGB6 J0555+0304?è‡Fî(o"?ÄL
6?Ÿ#GÁf<\?žVݸý?Éþ{O1{é?Ã|âýÁŠ¬?â
ô£|~'?ËKÞ/â4?Èy6.èTÔ?Çb'qˆà‡?ÏZ÷C%±%?ıJ‹?àoNLÒ@?³Sæ0'
"?¸]ý»}z?žî'UÑ(?Ù
&쟊?±Íîޞ}½?Ñ»½.ñÇ?ªéá²Xý?ÅôՋûýk?®I0Œþâ?áÿl¾i‡Â?³ãؘ'˜°4FGL J0555.6+3947¿Ü†_£@&7yéÐêÀ8ÃÑv¹À;™Ø)!az@—v³·X@-µ@å£?¯ó–Kwx?Êe*&D7g@Á+àŠð@$5f¿&Ç¿ÛMÓÈi½¿ã½R ^DY¿ê¨ðN²¿ë-€@Ø¿î9Ìzd¿ïÿþó…õAGNfsrqB2 0552+39A?ïwä
ëú]?‡Ox
ìãZ?€)""P?{¡ãX`3\?iû[mÔ¦?}dÄ;–8ø?îØôx§@?³-¤¾©%?}oòI_›?•
°Öð?«rvì`
?²GŒÕy?ìªl±Á¯Þ?¢ãÑù·è?¥×3;›?—_<­ÞÄX?¯')ܱÆx?˜Ãí
?1r?î—hñŽÞ?Š Œªê?—ˆ†œ>-?x=á_zåË?žG8þ€%?"}7?d!4FGL J0556.2-4352?åƒPàuÔ¡À;ö:\`‰À:&þìɹÀ<G|¾—ä@Á8jª™?ýª½þÓ°?¹œµØ¿tJ?ÄZã»Ñ§Ó@	®¢?Zˆã@	茿ð?ð¿ÑÄLá<P¿áânÁŒ¿ã©LŒ ¿è"¤o¶AGNbll3FGL J0556.0-4353SUMSS J055618-435146?ïòýüñً?PØ
Œ×Z?GDÔ‰e?C*Œ8y
?LÃ8Ï?ER	÷8?ï©ËòßPz?†•"!u?@"ž9Ÿ?W€©!cÓ?"Œ{aýÏ?…Ÿ‰›Gq?îþ+¾¨ÿ"?…"ԗH\¬?zr­•0»Ñ?u®"D6w?™Üœލ?€¸˜#QÞ?ït¦Ü捵?t¬WÁË?b#ŒÑÛ}?R­Þçõ•?ŽMe'?rúJMó¥4FGL J0557.3-0615?Öтéÿ¹À-ºIÂÁ±À:''¡WÓüÀ<*ý"û|ä@!7œÏY?ÿ—{ž?ÂàU*S懿t¼™4*:L?©¦^ÄԎ?ÿPûB÷?Þ­¥,tÓ¿«ƒÕü»Ú¿èí±´B'L¿Öð½!´Õ¿á,ï¢9Ñ2?²¼ŽŽ#AGNbcu1RXS J055717.0-061705?îÛ½CšÛ$?—˜E¼Ë!?[s\=á+?V™s¸?¡kX+p^·?—hh+?îæÝ'
=«?§ZÖçU?Z¬|'Â?h°Ð<™? ÁX+Hb?¦'1bލ!?ì¾8¹{HÈ?+–ð¡ý~?€m^cx{?mIo—
?¸Žg¶·?›v·ÄµQÝ?ê9§åI? árû@Cx?Š½%ïV?xNyo¼íJ?Åxg_ߣã?¡<é֒^4FGL J0557.6-0721?ï¦KXÃæÀ. ù	kºÀ:ÔdÓ¿/UÀ<@Ñ0ߛÜ@!GÝcp?ÿ¢ºtÛt/?Èêo_‰Rz?Ê¥Þ©÷"?ÉU·­¢@ÂÌå¤?î¥ÉB©É¿Æ3IÃîVà¿ì"֎ín-?¦ùQÁ¿ßË¿ñò÷¿Í9б3AGNbcu3FGL J0557.7-0720PMN J0557-0719?ïk‹%éy?«N¯9
G?;ó~T"Eæ??ڊºìe?'/à¡ðƒÍ?lŒp?ïªÛ+Ð?Œ"<+?1lqæ¼?E¯_qŠ£?"À÷ѓ,¨?‹ð"Ò<äÃ?í‰9'.ö?—
±ƒ"?m'¡ÔØ¢?aO¤[Ü·?²Ìö_èÓA?–K[‡»?îÑå~±2O?‹;bw«²?]½Ì¤Z°?U(÷@†›?¡ó¹´_¸<?ŠÃG@ÌX€4FGL J0558.0-3837?ïf™UbCRÀ:mYėtÀ9¢&¶ÁÉÀ<.‡'§
ö@ʹø´²$?ýnz[æ±?³Ò<^'A?¬Ü	֘}?ù&رÝ]@4hwä?íCy1DEª¿â$;H«j|¿Ü»µƒ+ß¿ÛÕгÚ
¿Ú/¡ãêöƒ¿â¤®ÀÈ1²AGNbll3FGL J0558.1-3838EXO 0556.4-3838?ï•àY|ý?y½Yˆ ì?N"rh뮐?A\½Òv…?ˆž¢yÀ?~VsáÈ°X?ïsOã%º9?Ž5£\¨?KÁáAÏY¢?`÷‰ˆ2µ?·ô':>;?Œ@Ü[üî?훾—|?—t/xc
3?~Ž†ÌùŽr?q!ŸÂðú?±9&¦³«6?•¢&Wj‰?îAÛÙùm?ˆ]ÒëeNÃ?}žjQï?ft|ú{?¨:ŽÕ+<?†³è'O®4FGL J0558.1-2859¿âŒ}|W"À7™0ߛÜjÀ:Ñ]ÓÀ<šz¦]Í@Œ›Ág
@æÜB‹–?˒ºNðÔ?Æp˄£=\?ø™åi{Ĝ@Ç9©Ml?ïü›ÇqC9¿ã¥ÞPݾ¿æ4Š¡.8x¿åÖÇAÈwS¿ïüõ$®5¿ïف±E‡ÊAGNbcuTXS 0556-289?ïBâWú?²>P	
~?p1Ž®+?²FUÒéc?×8±Q¢?‡)]v1õ?î×55×õ?¢n1c‹?tupCÓ?‡æ»éœé?¥sì*Ôx*? (ÜRÇðL?íÑG" 5?'šâ±œ?‡ï°fu^n?wê'[i?¬ïš´_On?…¯ï´‹?î0%GB?‡¬"©al?ó†IŠŠ?rήCPë¥?¦ç)6?"eXš~&ˆ4FGL J0558.8-7459¿ï\nW˜åŒÀ=†r!…‹ÆÀ9҈u"ç[À<U¼ö•óó@ÚJŒÁo?ÿ¦>{f?µì>A¯!ì?±›!ô›?ûHÆÆ#@ê¬0Êù?‡'ÑTW+¿ãf$!Gx¿áÓ/M= ¿Ü+%Â1h¿âG¦Ý¤áK¿åW¥£"ŸAGNbll3FGL J0558.6-7459PKS 0600-749?ﲄéàµí?sŒ6»Zt*?MIo^@í[?@Ô4ºsv?Š.'îuð?rˆ؅#?ïUœËã±?'´¤=¹P?F+Ü݆?SDº*]G/?"›
Ä¢ï¿?'\žÓb×?ïAÈ3¿¤?€½%g߯?fèí\NG?RÐi‹ÊçI?šº©MþI³?(™\nï!?î–ȈîÞî?…Ðx…±^?vqìϲÂX?`5¿þÛf?£Å9׸Ü?"s—3ƒÛ¡4FGL J0559.6+3044¿ã™3·ñž@EF%~>ÊÀ:Òn`/ë€À<Gfȋõl@"iôÄb›?ö¯•Ôèû?ÐWN»¤ÜC?Ú¾•Û}À@
¯H<¯³·@0&Ø1¿ïÿ£ž\w¿ïºÔaì""?ïþØ
b?åƒ)ë‹Ôµ¿Ü=½zÊ¿Ûö]"ÛšAGNbcu3FGL J0559.8+304287GB 055627.1+304251?ãQ%	&Ø?Çã¡yÿÊ?™¶h,"?Ø?"?hjû,¾?×ÂO{+ŽR?ÇE¼UùÒ´?âq½"!Œô?Βrîï¡?—áLógÒ?°T-m™À?Ù¬'¦í¯›?Íkp‰ó?äjÍ°?±…È	+†?±;Ė­^?˜µžP™?Òê5
@%J?°#Å@å?æ݆Žü
|?¾'sÔ¹7X?"úÊW»{J?‡…Ë7֞?ѝJ	,?¾0—ï&4FGL J0559.9+6409?ØìøÛc
@2èß?–À:þ¿yýòàÀ<´ZÐ0.œ@f™<ÒnL@¸<½°Ÿ?Ä8âʐž?¢Û=º?á°ê7.j@ž ÀêÁT?ïlËÀ]RÁ?£î˜àJd¿éól|*¿Î7UAPu¿ÝA¡
&¿ç¬?8¥
AGNbcuGB6 J0559+6409?ï$w1Ê?'£A[zw?bÒlC%Ûb?UJlü-?™á#'b^?'˜ƒâ±õ¹?ïG¥=š?'¬TFÅyù?U¢&‰˜#µ?bjˆ™ÂD¡?•Ã;"¾Ê¬?Åb["µ?íÒð†ì¸?'¢¡qXÌ?~G›Vª^½?oXø2l'*?¯Œ»èÆ?°Ùvoëc?î—ô³PÇð?†'Zܱ3j?…ۏGâ?re‰–œë?¡@-Ô¯?ƒš9%l¬4FGL J0600.3+1244?âã½&ü™Àú¼þ"°À:$™Õ(»áÀ<` SÇþ@#^ÎÚîùr?ø4þ"ÅõB?Á*h‰VUw?ń8Hñ¶f@vQElñ›@–A¬rº2¿ïÿ='—t{¿ï=ÙìD?ïÿtµÍ­?Í'"™2§¿Çh—Ð¹¿ÞqG ¨"AGNbcuNVSS J060015+124344?éÛú¸X!;?ÀD!jåå?†vÌ^†Dv?‡‰ýñ4tº?Ç(¨X·Ì?¿vûm‡ˆò?áG"	G½?Ë6Æϲ®"?j'ÑÅED?'Y³_­ù?ݺKUååû?ˁ
:0?åù½Þ4,Ñ?¬'»lD¾?ž˜'êà(A?‰oeê
?Ò"û$é£Ù?ªéì"ê–?æ'ö˜Çœ?µ¡C؇#¨?ƒC5ªkÓ?å•ï"´?Ò?ùTaj?µ¦üͲ©4FGL J0600.6-3939?àe'潩À:6¦ڜ™À9Çü6FãêÀ<"š3Œÿ@»3j:±W@nu5¬?»S9¸ÞXe?ÉJ®yûn¡@'ÌÛæED@w‰µËÔT¿±gû;õún¿æJ	¾Å£
¿ë«ð«Ï&¿ëژÒÊ<пí¤Qƒ€R¡¿ïû´áô|>AGNfsrq3FGL J0600.9-3943PKS 0558-396?ëb"Ú	â?·ù_Ó\GÎ?´Ol?š Ä?ª`2dHVª?°Ÿ|ðð*?±Ì`¼Þ³?è싃c¯³?ÆÉ[nè\,?¹WR3,ÀH?Á	~c)?¿DQ±µÂ&?³ÿ3\*Û!?çR
•3ùÁ?­Ü‹)iÓ?ºK¯s?£Õ³‡$|r?ÅwLŸ
AD?¤'3ê½?ëÚH½ƒá? ÑBÌgmÒ?°ìD7…f?œƒ¦T":?°A{BŽzØ?'½¶¦î^/4FGL J0601.0+3838¿íՙ̼@›%,à2ÛÀ9{ôörÀ;ýxM·‡@ 1ÊRt?ÿHécˆÖ?³«½ž¹þ?°ўî˜$?úkIÅEïÎ@¯–×óF‰?ïð'Þh¤¿ÖÊ'¿âµŸSí½Þ¿×l=Æþ¿æ·E¡ŸÍe¿ÉJ›Ú'†{AGNbll3FGL J0601.0+3837B2 0557+38?äˆ×$ö«ß?¾®Gˆ#}?Šb—‡Âu?"&ÜÃ.?Ö<ùԔ—?¾‡¾>\?ÚQu¦Í-?ǑÝíôî?¤['vŒžB?®ik@ªaµ?ᑍ0´†?ÇÂ~±—Ô?è:ïÒ|i?§EO?¸­|?š'ÏÝζ?'ÙÌT#D?Ì ÚDü7›?¥w1ÐĔ?å§ÚÃ]­?¨œ®±ÊM­?·n¶il¯?—.&Kµr?ÍÖ^-½Òõ?¥ö¸å®Í§4FGL J0601.1-7035¿ÃhɁ)¥À=¡g‡Î•ûÀ8¹£¥Œ#À;è×Òª\@ñe¸°–@ƒ‡Ä"ÿ¯?£·¦J*ø?½Ò/ãšj@Fº z^k@pM6>«a¿ºŸ»Ç–×ó¿à*Iëœø¿æÖ`)5ƒp¿åЬÀ½ÊÑ¿è·âŸÇÛ÷¿ìT*Ÿ:î>AGNfsrq3FGL J0601.2-7036PKS 0601-70?ï[ÄñVß?‹àýƒ´—?m=p+‹?uØdô?•í?ß³ÏÂKˆ?ˆo·ÀtÈ?ïÂÖpÐÔ±?~
õÐãmF?2ø0}3d?DöäO ôˆ?}eDÂv?}õÊw§?ïK@‡Cîý?""!‹Âÿ?pÛ?µúqŒ?ga`¶ïzh?'a*"&?àã÷0?ïêiCˆY;?Rµúüí´/?9"¡*áÈ0?,̽bþF°?brhRJ‹]?QI[Ï&¢w4FGL J0601.3-7238?éázÍëI©À=‡·Ïå†À:øz§fÀ<£ñà'Œ7@\\sôC‰@âÃäƾ–?Ä wÚ,0à?§—j•J?åü~ìC@~q'´¿ë[þ*?ïô¤'*è¿ä?ʅʯ¼¿æ«QAç*¿Üá-â'Z0¿Î±k

pAGNbllPMN J0601-7238?ï¾n¶™"?t9zqF0D?Gl-vH¾o?@Ž1-NA?}Û¥æ›?s¥Á0$Ø[?ï—ÚõèŠ&?…؈jäÀ"?3ò^ÓQ"?Gü¦°º†?‰i¯Bí¼?…:J^~†?î-`¢Ã?Ž'nIó?vž2¾62?cǘΒ'Ù?ªV-.õ?‹´@·
†7?ïg–Êi?wbLj…K?aîä?Tjº‰ëš·?Õ×J?19?w]0HíLs4FGL J0601.3+5444¿[`§݊ë@.=Ö[æÀ;7z)'ÉÁÀ<°œÉÏÂK@ Ñ6Œ.!&?ÿ€ì#ª)?ÉÝÂéI/?£Š¾ú?Ùb2z&@gï›û2?Ϲq%\0¿ìÕSïk]F¿¿c"OðÆ¿Û^'¢O¥¿ÛÞ9¿ëížÔkýAGNbcuGB6 J0601+5443?îͤA¤?«>¨W?\u¯ò¬š±?Sÿ¦1n?­úÕ¦&€ò?«pЖ?î%^õåÁ?°K–ñ-Jþ?[¥ýDÓÂ?gד²êsr?¬Í©Ð·}O?°-˜^mþ?í‡Ç/<µ?–Œ
"jJÕ?tï[µÁ(}?aaAfI?²rÐÌBÍ?•vûοš¢?î&jò_Õ¸?kȗ#"?e‡¹å
š?Tàâ߶‹?¬@ß~dS™?Ú•a4FGL J0601.4+2320¿Ó-CŸççZ?Íb±%&€À9Q¡/À;?‹!0Ò0@Ò.ϏÐ@#ë¤ÿ(j?Ãðç^HŠ³?ÊÛ9·†¿w?ÿãÿ¹‰#*@©5§¬¬Ç¿é¬¤G¿Òvǝ
"¿êçÓh'1¿èá?(‰â¿ç)\OŒ/N¿ïã²…AGNfsrq3FGL J0601.5+2309MG2 J060149+2324?Ê¥X¨\ƌ?¿ýÚ/÷?–Úf'zô'?"',XÏ:?èŸÖ¡Tö¼?ÀZ_LYË?Òڒ̛?ÉÊÓV^Eý?¤à\G?±"¨Mc?åQðŒ³?Ëh¼s^Ž?ÕPÂ1ÞûÃ?­õR ?¸«wîÍ2"?™ …Â\"x?âB/é6ÛÍ?­¦¨€6z?àuóÈ·'?´y¨9
	í?±Ž6Ôý•?•ƒº´é1.?ÚÌ4àܵv?µ"ÞÁFò4FGL J0601.8-2003?yïÛÀ3Ùä"sÀ::Ó8÷˜RÀ<L•òE,Z@±y]äâ˜@ir)Zl?ÀÏÔ©É?Áª~™8 ?ùA".öŽ@ÞR}T•¿Ï®2M"¿â°FŸ ¿é›H€w^±¿ì|¿8"†?§"Uür'¿ïýïŸ_¬8AGNfsrqPMN J0601-2004?ïàº-üÞD?mÕPU™äà?MpÃeñ#ê?P¡‰ò¸?gé¡)¥r•?j+Ԕ£#ú?ï«Ê³öÝY?Š©ÜQ¾vâ?AÝpö3"r?^^-¥ÉK?ƒï{òåq™?‰ž¾"?K?îŸ<œҝ?D¸XåL?pJ'We?h‡3ä©r?¤õ/kT?Þ®âåÛ¼?ï¹é÷D–õ?lO!¹måã?FÅ*èù-?A{0iìV¢?€/€J°J?k%LgÕÓ54FGL J0602.0+5315¿ïŸ;˜m°Ä@-%åр´À9{ÌÀ7"À<+6
Ä@ÈÏ»i£?þùLVè?®°ÀÁj‡Í?œt2¬Ðƒ?ð'޻♾@'Áƒ¢?æZºÌH¦¿Ô€'ཚ€¿á~•Üär¿Ù5_Þ7v¿ážXæK#¿ÓÂùå3ËßAGNbll3FGL J0602.2+5314GB6 J0601+5315?ï¸Í ý¸ô?€±Dh^bh?89àκ?1—szL7s?ñìt?€bC¡z%?ï­hÕÄ[??…Ý|ß5¯?:À²•¸U?Lç°ÎÀÃY?ƒÏÄú;oQ?…7R5ǜH?îòÝJ¬´?†n{)†(ê?jdMÀòº?Vs|M	f¼?žWÖŒo?…'Ëߺu°?ïp;l¶–Ò?v`F¨½<?bßÙé"L?Kzüu4?l¬ÛßæR?u$­«q0Í4FGL J0602.7-0007?ïáÓ¢)
:À%»Åޜ*À:@x
Ә™À;Ê%o%QÉ@i€0¼áG@S7ë(Ø?Ê$ Eűû?ÃU6hFæC?ô²—,Ê@ÏÁZRÜÇ?æäíU'¿ÒãIüMmò¿éSe¢òð¿àÜ®ÙÄ­¿çãœA¿'ý¿ïÿð`OËðAGNbllPMN J0602-0004?è
wÿþõ?ÀËmYç?™ý—KÐÙÓ?­à.Ž‡­?̊m€ó?¾ÝLx¼éP?ãƒä#õZ?Êu½îˆÇM?•l«ÉÝr?žR]>½{»?סm?&7u?ÊÈ!ðÃ?äŒ0¶"4ï?²þ)g,Â|?¦m 0¼B?Œû2¸ö˸?Ôꍤ?±¼¥ÎDš?ã!€—•4ó?©FP_>€?±I'Áòà?• (¨O"?Õjš XÞ?ªGCÆ4FGL J0602.8-4019¿Ôw"¨qUÀ9÷±ÿÀ9HÙè>B[À;֞-}Í@MË°4z?ü¨zd×ñ?°ûe€Q7ð?º‰Û
¨$¢@
MÆýòÿ@çÖøj¿ïá÷ ³SÕ?ﻹ.׿àƒËÑû	÷¿Õ(šž&q.¿â«¤(hÔÖ¿æ &5AGNbll3FGL J0602.8-4016SUMSS J060251-401845?ïIº"?"£u2ðʧ?e/â5Â?dœ]ç$gI?†¬…~ú+n?ÕÆcR{ƒ?ïúÕ¬˜‰?™uJõ/×?möÓék{(?}M<5`ò ?›!ÊÍ?ˆ?•ÝŒ<v
o?í@Ø;ý»?ŸQ™Âƒß?ŽÊì¨uh?ƒÃãÝ*Ûü?²àž'»s?˜'ÍšžT?ì›0	ï¥û?œ÷ê²F?'}2÷ÄÂ?}'î9^§¢?¶‡3,ÄÞô?›ØU{ ÊÚ4FGL J0602.8+6041¿å†¹'³Kq@1ÒZh+b"À;LN¢ûB+À<›—¸
@çט'Ã>@k¦ý/k(?ÌȆŽàÙ?·sÞt?î'ÿú Ã@p ó•Žr?ïØ+oðRä¿ãDD¾ÂH¿çÂ>hñ["¿ÝÛ«aïÿÿÊPË?ïÿý¡UûŠAGNbcuNVSS J060324+604009?ïŒ=¡|v¾?ƒ&MŠK¶¾?c¡:Jì{9?\¸:"Žk?ˆI'1Û?Ñ\™ØZ,?ìåe´¡?µ»GXü?Œå÷jà>?˜;¾Td­?µ81 òð?²"ì.wÇu?íE¬y¤ž?™Y<ˆð"Z?D·ï"›?C<µ~8¼?²*€ìèž?•ª§*H?췉©Mô
?œ~ªÿ0s?Æ¨}¥›?}žAƒó´ñ?¶ŠÝ³ªÞ?š…ƒróN'4FGL J0603.9+2159?íU`U³Ä?¨˜,C;À9g l‡ØÀ;IéÁЈ@‡T>7É@·a*½C?·œ8°J¶¿š€)†G\?ãA® 9[k@	 ˒:*?âÁ?/À¸¿âÀ+i:V=¿ë¦¬ÂkIû¿Ñö0‡ÿ¿ëÄ®…¹èÄ¿˜èíû׸tAGNbcu3FGL J0603.8+21554C +22.12?é\ý_Rq%?ÀE˜ØKê]?{Sˆðìl?q—lçpV,?ɳWæn´?À؈
a$?æ¨o'fx?Ì	ā¡¾?a"¸L¬?w勵¿vÑ?ҍÁ‡Âx?Ëè¤
Î?ç̊å«é?¯MîKzG%?¡A8—9?'¡±îîÎø?Ì}[-ôM?«âŽ$È0C?ë5AQ]§?¢¯äpï¤ô?†=
=?sråȵÈ?ÁɊ¶1H"?¢6KùÑ°4FGL J0604.1-4816¿Ö[YÆ"—7À;}Oß;dZÀ:‰øg…JWÀ<|õÎMÖM@!SCÉÙR?ûêï,s%'?¿÷>….?³Íï6¯©?öêºÅ­@ú9lˆ>¿ï°OžMÞZ?ïüÅþ§e_¿ÜÀæå|ǿ܍üb;´a¿ÜÕ9BkàN¿Â¨Xú2ÍAGNbll3FGL J0604.1-48171ES 0602-482?ïÙÜÜ
"z?k'»UIâ?6ÄpÔÑA?00!X·'¬?q¨…³°uï?jóå³ÅF?èëS©?…©¹EÅ?8ԇ8ý=Ç?N†Ã¹éO·?†á‹c+°?"·4Že?î½½a4°?Šx`ìÄÎÏ?gè€zc?S›c¡ï×?¢³;d­Y9?‰†8³ÊÞ?îÀPŒÛY?…nqÿ›×¦?j5ÇäI??Xdõ—äo?¢Wž%Ì+K?…Q¶È@|v4FGL J0604.5-4851?Ò­Td¹Æ"À;‰¹"¬TÀ;5£ÇeÀ<šó5í"@:^}¹¿)@{\ÚÌiÐ?Åícۜž\?‡5ÖP¯	?ÁÊ'˜˜"@ftá~_¬?ïõœdO4ñ¿å›	Ü!Ôf¿éë‡ç`Í¿ÝÖÚhµÌ¿ês€€C¿»4.A2³AGNbcu3FGL J0604.7-4849SUMSS J060433-484947?îbZ}p-'?¶÷܍MLi?né
©:¡`?jæßÎHN?§ëÇ~iƒ{?µFeΊ±ø?ïPŽ¾þ:Ô?‰N¸Èi?LùVí!©?^Fšì/?•\%<}?ÏȶrøX?íë̘a÷î?'vÿ§Ë?vꯩÙã®?i#þÆYË?®eà"¥D¤?Àbkp>
?îûY‰ÈŒ•?€››MW?fú2žp½?RtA,ÔT?µˆs U ?€˜­dØÞ4FGL J0604.8+4411?ß/썲[@%Èù±1eÔÀ:ecãÔPÀ<Ȓ«hÏ@:"çÛÇ@oê#èù?Ã×ã–½Ç ?«M-5?åŠgAؒ~@˜Õl²?Ûú"•üV'¿æ»`(^ÃÛ¿âèìô,¿ê§Š$Ô¿æ²^âc¿ðAGNbcuS4 0600+44?îëgð½?œÃ?)Žë?g²Ô`
ۅ?ea°ÏÅN?ŸœÄuý¬ô?›¶£žÈÖµ?íÍNçD2?¶RÔ&…ñU?`@Ǒ1~é?l>ŸRsX?±'‰Qòn?¶»Åá<?ìùK+çã6?)Ý×p^?ˆ/\Ô?{§"Çc?µ2À¯ú¹?™¡7í˃V?î^֔2"/?†>Ƭ/ê?x2Išq"?bqrÁTž?§s£~ô?"î ¥Þ`Û4FGL J0604.9-0000?ï U'¤´«À$§ñQçSÀ9Ö¡Š(ãNÀ;ëŸ+©Ñö@ `|°Ä®?þŤðñ5?ÁÇÓ(["Ð?Àöh½ÕG@Õ%`â™?úé!>"l?ȏËåq3t¿ãP´î‰µ÷¿ÛžgŸ —$¿àÕß?Á#¿ÍÎùÁ¢w¿ïÿú Âî'AGNbcu3FGL J0605.0-0000GB6 J0604+0000?ìX͎a"Š?²¥!^þLý?yÉ=ƒˆ¿í?s50"cÈu?»œÿ´¾_¯?²@mÐb§?ã^AßSw9?ÌW¨ÄÕ£?'¨ÓÛÝQ*?ž¹¼ù+dä?Øï›<{?ËÑÒ±È?è·7€¢?¨`@E›Z?Ÿe!¹¨?Š0_÷ÈjE?ÈÙ?njÈw?¥TXºù*þ?≀–]ö?­QœeÉì¶?¤™øÛ®Õ?' šúVÁ¬?Øk‹"*d:?­½¤&"4FGL J0606.5-4730¿ìßÄaøÀ:ò|ᛑÀ:iƒ¾f½À<~)gØVn@¹_÷·\"?þSó?ÀgX>Zƒ¯?Ä5â:[€@Jb#ᆘ@ÿ8¯ÉÝ¿Ê~ÆÀï?ï†va[9¸¿ØBµ<u¯¿ÛlÛ z3x¿ã'ÿýPοç¸u'8)AGNbcu3FGL J0606.4-4729RX J060635.9-473001?寮Ï.ÿz?|³3þ/m¿?jøl|ç?jù-)CÈu?%b"ý?tÖ¿Àۖ?ïRîïhç?'ÖË£‹¡?T*ìVø?aþֆÅÿ,?"a_Ms²?'u·Ó"e\?îÆ\¡¸O$?ˆ²:7D‡Q?q;ò7P'?aƒô˦?¡r·'Ò?†sÙ2LÓ?îTnRI?‹övŠ†ä?ŠùÎd—?sU‹˜'V?§óºªq×Þ?ˆ	ocè*¨4FGL J0606.9+4402?瘝wÁúÙ@&SZBkµ[À;ˆ²køvŸÀ<¯
¾Ÿã`@"vJâ§T˜?àÖ`ÿõE?âÌ|ý?ïÿÿ&¦³@™xâií@žÔ2FÏ¿ì?2_Μ±?Ûìû@}ž'¿æïa¢1n¿Æ`¯Z9²?¿ÒČ¿ïÿ̞©£ÓAGNbcuCRATES J060650+440144?î'9š¡‰a?©+^ÛÓ¡?Œwø'Ý7?žÛ¢µNŽ?Ÿ|Ðj`8v?¢J¥,y?æ6uí?Òw€k£<f?""7»g‰l?®«^vb?ÒJƒ˜ogh?Ѭ3AJ'§?ì.…»ªge? ‰Ký—\?˜êl'Wc³?Šwñˆ1?¸Q7ëñ?œ
H2â?é¼;½ÿ‹"?´î08¹?`¨ü4wû¯?pèâVT\†?ÈÌm/ò?´çrñ œ4FGL J0607.2-2518?æêÐN^ïÀ4mÙ ð¥ðÀ:ñe9?¼®À<­¢pØ°0@ Iý?üÿ¥·µ
"?ÌNÖý¨7?ÒûG¿1X¾@*3<m@î" ÞÇÌ¿ïÿÝÑô?ïòÑ®³Ý¿Ì°B'—É‹¿Ô§â݅W¿è…ÀsοÆx øóò+AGNbll1RXS J060714.2-251855?ï³M|KŒ«?w׎#Ýä?c¯óÍ_©?c‰Y5PC?|ÊiàRú˜?r`7Óâ"?ï!Öz¬Wª?—YU6'¤?iECzc¡?u@MA|È?˜œˆ;(–?•!¼f­%Î?íh$tàÑ»?•ÇT	[?'/÷øk¼?ƒ°`þTt?°rÞZõ—??'LS¢kb«?îCÂÏ^Œ?ˆßÀ<uMq?‹;ñQs;?t!UÐVß7?¤÷'~Æ:v?…!ߟÅ	}4FGL J0607.4+4739¿ä"oLi@)»ZBkµ[À8KÅPÉÀ;‰†¶hz@hÛ!yL?ÿ묋å?Ÿžöaù?²î˜àJd@Éé^ÓÊî@€9Küï?ä·¬ÿýѧ¿Þ­€×*ô ¿ß–7D9ë´¿Þ9p¤'Öµ¿ä,™¦5¿æ%¢HZãAGNbll3FGL J0607.4+4739TXS 0603+476?ïŽËAuƒp?§h<3G?DÑøÞði'?W6Áù?‹°H?¦h"ôj-?ï(qÏDò˜?œÙÃ[Àä?e¤#øU??tÜÌ¿]&Ñ?˜=Dâ¢G?›ƒoڍÈ?îô•³Æ]?ŽÝ"ôÜ:Æ?€"£!îCÆ?|pßN÷?™[÷ö=:Ÿ?ˆWÕCI=ë?îËÃé©?‰œzäþƒ<?{›õ|"?eÛ` ܆á?£±OMµÝ?ˆÑQºËðJ4FGL J0608.0+6721¿å/"ƒÁQU@4ßH!ÄvÀ:É¥Ð߁À<rÁÄN¯@Ô®rC¿G@e²€fÃ?·_ïÕ?¶O•¿ol?ýŒð=ë@‹ëëv@?ïþ¸*¥¿åڀ¶–*¿æšmÔﱿç
ýQúÊ¿éOt¢>XÖ¿ïüßÿÚkFAGNfsrqS4 0602+67?ïèahu.Œ?bÛӅuOe?FÑ,Î|²
?DJƒ4±&8?aêLW2H?_I…ºü?ﳀoœ ?'*åÛ*[?E"vèv‡?W	r¸ï=»?ÆëяS?€ ²Oż?€8ì?€6†5QK?rڈ?k €ÞÔ?——æ´L<Í?{šÕÂèU?ï·~ƒBTV?h<=ª¯¬?d
c_i?QE1Á.šû?z3¶X$%E?d[Cþ¡À‡4FGL J0608.0-0835¿áX¢X…À+-{cM­À8z!ÛòÚÀ;gUá³äž@Vä£-@ÝÛ?VW?§ åþ¢û?²#ì€ÏÚ@M­àx{<@­þ/Eh¿É]úºpª¿áé1â¦'ò¿å¬¬›ÔÝ=¿år|õ$®¿ëÏY¿Žö¨¿ã‡%Ž/AGNfsrq3FGL J0608.0-0835PKS 0605-08?ïq»W]X$?†pïZ]°M?N8YôZ?F³¬—>¹?ÖÔl+ß?†¥Ë¸mé?ïÕ¡yéO¿?{3zì‰W?0)R¶ÍZ?J΋á)ç?t,«,³¥?z¦ÏWºŠ?îN4çV?–ÂG¿Uƒ"?Š_%Q÷ý?…@í(¬c?¤sôõŽ?'°*Va­?ïÅöM$€Œ?f\¾¡ó??¾SSd;«?0ÂAû¼e?{ô8‰v,?e«C]dXW4FGL J0608.1-6028?è:ñ"½aÀ<¡ð†nDÀ:+>WS£ìÀ<
¢"ú¦$@Þ)=Ðñ@T™Â´E?ÅÆæXäóŠ?ÇU¸a°Ê@¥á¦x¥@Ô&Z²©
?àî姏&¿æf¬![š[¿éq+¼FlÌ¿éê šª;¿ïÿøþÙå9?äãÀEçAGNfsrqPKS 0607-605?ïäºêà«?d}›ðÞä‹?U¯¨ÒHû×?O³ÅŠA?`mA'úÖÏ?`4x¼F×?îã׃Ä?ŸÙl$ò"!?g•Tߨ•?wkj-¢ç? I2€ã"Ì?œŽº;lÞ?îQŒ²¶K?'§('Ïý?'e¯š#ÈT?sJÒ.Ù÷?¦M›NK©Z?(À™"º?îó"Gb²m?…v~‰Í?tÒ°Li?a"nA?œi¢g…ŸZ?"±ØՂÆ4FGL J0608.1-1521¿ã~GÐñlÀ0aóFí$À9²L‡À;ãIâ¢!@ª<ANÔÏ@aÏBÈÒl?­Q4¿¿	?µåê**ËÜ?ÿG±õ°ñ¥@ô÷ή#i¿ÐFŸ ¿â-¸À%t"¿é£€}"Ô‰¿æ5v•ˆ"¿é"|žâê¿ïÇõAàõúAGNfsrq3FGL J0608.1-1522PMN J0608-1520?ïçajb\?`=íà/ÃÉ?;å°]p?1ëÖ^×F?e!ߒ.¡­?^رº5…6?ïنœLÒn?yžv¥-^J?$Ž³UÄNi?;—ÊÍ%
?r˜<>è¦H?xÙø¿¨ë?ï
£fæÂ?ƒëªGÑ?q²ï:ØG§?d%°íò€Ô?™ÑïÄmÂ?e·zº?ïïvj=S'?MZ&§ù½?1GÓ
ã7á?#LÇF·‡å?\Á6 ?KÄh¼5;4FGL J0608.9-5456?éo-&Æ`À;Þâ¨dªÀ9·CsóãÀ<^ÄÞÁÁ×@Û]ˆœFG@""³º­?¶æPV"œ?Ø*ƒ·/,@ö"aKts@[ûÎíäJ¿â F\㕿ãíÝÞÂî}¿è\…qÄhz¿ëZ}ú×¢¿íÓø:8á¿ðAGNbcuPKS 0607-549?ïð¹‹b?r؈‡…@?G~z"šÀæ?WÇȐù?SAP»›Ú/?i°nº€"?ï¥ßnoát?ˆ6Õ
‹k?Ciíí€?`Bè#Ë-?…Q"e(ÊÞ?…±Ø	D?ï,<õBP?'ÿ>˜Áp?rÁñLüd?páVü?•Çå'€-?€F£'z¨:?ïÎ_›²œ;?e.˜¹R)?b'-dïg]?S	¸1ñóÓ?oy6èt]š?`´æÐ.ð4FGL J0609.0-2219¿íTÊM§¹ÔÀ2ñåÀ¹™À:ãêÀӚFÀ<x
œ;4‰@õ¨ä_@'‹vÁ?Ò:og–è?Õ£(c¡e@°ÄXŠÑ@	ªçŸ¶ê?äEôî¿äb¼ÃjM|¿ßM<+¬¿á¡4x­'¿êƄ^I¿ß·$¥Ñ¶AGNfsrqPKS 0606-223?î•sÛÑ	¢?™GΒR?w7"Ž¶vø?q#‰¯}û?£Áϱ–û?–ÿy2lŠ?îżô3"=? KУ³?qNn‰?	ݝâ?¡€ù	n?ˆÂÿ½Õ?ì¦þñAü_?ž2-ðP?!Úv~î$?‹4¥¦+'Ž?³'ØPa€?—îÄGMK?ìï@!‰z#?"ÁoÒ©]?}2ú;H"2?g¥Ÿ=²*?¶²ÏOÿ¥²?"¶-è5c4FGL J0609.2-0247¿ïʋDþHÀ%Q|=h@[À9‰PÉSœÀ;Êrß­*@ 7QŒºŽ?úºܓn?¸õÜ»'M?LJeºnü7@«3¥Cò@˜¡˜–N¿ïÿC*!<?ïýûþé‹¿¦`ʛK¿ÔŽUëæοÚbX"üS£¿è'kr>á½AGNbll3FGL J0609.4-0248NVSS J060915-024754?ê"{U)?»M+{Ê<?«N
«+Ã.?¢.xÃ0ì?ÀÆj§àk?·bÝa÷Or?쨞ð-Ö?¾m™y?"=d"/Ո?¤Jíaóe?µ°	ÿò›ç?»IqΆM›?çSúZM5?«Ð'øý˜?µYT²?}´?¡Êèïo:?ÈM½wS?¥?
q»hæ?äŒ÷Ÿ¬}­?²o×Ö#®4?¦?¢D‹_?"ìoÂí@"?Ô/Ì^s:?³EñÝQ³›4FGL J0609.5+1402?ãÊ­úí$À&ü›ÇqCÀ9¼ˆ\ZsêÀ;P°Å/Iš@×r'¦
@.—ÂÿÄq?Ëaë¼?ÍÍړßÆ@yŠ˜?ûptgÊ?ïkcÉ€?Ñ´GDãù¿çt÷Ãñ[ø¿éxv¾ù$š¿ãºàŽµ:¿ï÷šÁ6ì{AGNbcuNVSS J060922+140744?ijÔñv¾±?¶–sAh0D?Œ~bYÕÁ?åCmØ?êaºèý?·iºÆZ™?ÉÙyÆÐõ!?»ËÒ΢<Ë? »Ã
nÌ ?£Ó¯ók-?è}å]¤Õí?¿Æd¯æ~?Ó½­ˆ*™?¬?u^£Å
?¶"Ÿ³ô1h?–!Äëu)?ãNµEl-?¬améf–?ÒïÃæøf'?¨°mÁ…Õ?¾p 2îà¹?£éu'·9W?âº
%ð¨?¯èhEÚ:4FGL J0610.1-1848?êÓzóùÀ1Sü¹#¢œÀ9Ü36ÌEÀ<(!à$˜f@Ž±¥ÿÙj@SI€C‡?ºbe¥Ì,ê?¸NPº*?ýãGG½-ó@
âmúy-¿ïΣ Öå*?ìû‡_Û1ê¿äßzïŠf÷¿åu{aöD¿å©ø¡çÆοïÿ"ÞïAGNbll2FGL J0609.6-1847PMN J0610-1847?ïê~0N?\Wë#kí?CiÀ¿ ò?A¤ÆÐU–?`§_Îéý?Wò¡C"ƒ?ï¿Ê1(nl?'v'5'vc?9Äù{]æÄ?Kë'²J?~~—ÔëŒ?†>ÐôIÄ?îÝààk_?Šöù\†N?x£/OäL?o›AÇ]T^?žB‡8›2?†}½Õ' þ?ï\z›ÑýÓ?vIH,P¥?x`C¯æI®?eMa¶ž…"?Œ±73fm?q'®:eã4FGL J0610.7+1656?¬{ïñ‡D¿ð%Q(ÀBÀ9&ÞßôǾÀ:ù^³ê}¸@ÀØNá£@6þ.n¨T?ÏiE~d^ú?àó°0´Ó²@ê¦ÒgA?ôWTБӿ̼°à]"p¿áO^AÔ¶¦¿ê¨ªxäî,¿ë6Èéé¿ð?èÞ¸AÐYõAGNbcuMG2 J061020+1701?Ï•Iý3?Ãxȼx€?ÐâBi‡¯?Çm8´Ô?à8¹x¼Ü?əsVr`?¤,F¨ ?­ÁR5'¶?ԕdDšyf?˼ðjqRè?äsëHAM?ËàèoÿQ?Ïk==	¦l?®íËTü:Ù?ÌÆ_(tåû?©6\ñ®T˜?àó˜æ \æ?°'¸¿‰u?‡‰*1‹Ö?s6¬œ˜?à(îOç™?ºù÷t/ ¾?ßdÑÓÒ?ºˆÒùñ`@4FGL J0610.9-6054?qgTÀ<TÔÜeÇÀ:Vªñ°±äÀ<%ÚV"K"@Ës0yE@|#ßÙ?ÂMò?¿1ãÁŸ¶Ù?ø¿}Xñ3@
5¨µv	¿æ5(¡ù¤¿à	+ÝÔ\
¿è'Bbûù¿èG"žy_¿å#—´½¿ïÿ¼C͈AGNfsrq3FGL J0611.1-6100PKS 0609-609?ïòàÑ1Kï?S'ýÚ5£§?2=_£7H?-¹ýÉãö¨?U¯´šc?Q¿<dKm?ïaôJ™þ?Ž[Çß>Öø?J"kÊZ?`æ£ÁQ¢?'ìÖ©aê3?ú'®ä—?îüÃ*ËÛ?…dÌN8X?mAú o??\¹RB(?œ¿[{¸œÇ?ƒ»¾ùôž?îàcp_^?ƒ/"¬ˆU?q<61h±?`TšÔ¦nÀ?Ÿ­³Dg¹ì?ƒ?êsþJ4FGL J0611.1+4325?ïëÛäJu@'"ãq*À:ù»9À<Bˆ4ˆ@ «*èáÖI?û¬½³TUÃ?ÀA+‡‹O?À`Ò}»ÂŽ@*§Xžý‡@÷˜OŽ?ï9Õÿ{u¿㒰qLsv¿â}§Ë‹"-¿ÍzwëI¿ßõu|Y¿Û­A—$AGNbcu3FGL J0611.2+43237C 0607+4324?ï.ùpÛe?ö"Io@?e"L"P?^-γë?—í¢©ÚÄ?e'fý;©?æ±v©ÞUQ?ʆí(èÛ¼?Œ·µI'Om?"¨[5±u?Ñ·Uúâ?ÉþÐ>ÅE¨?ì
P/Ü?¡[¼JÍãˆ?ŒÊ›‹úPÄ?|(zÒ͆%?»æB
??Ÿf-¢h¡i?éÂá{·S? ™'	ÿ?¡À€ö¸{Ä?‹?fŒoS¥?ĄYÓu¿Ã?žÅNs®L4FGL J0611.6-2712?³*Ù"­À42®žä\6À:TWLíï\À<~vQ•ôÉ@®Š5x‡Ñ@HÜè£Ã?ÂE³ÆkŠ?½DÙMäa?÷Và·e\@¨AƒMÓ?ïÿÂÝ_¿åeƒGG½.¿å»;ÀJˆd¿äꨠÀ€¿ð?ï©·¸iAGNbcuPMN J0611-2709?ïôû&æ?Qо.>qÖ?$Ýݕ}?#b&—&¢?Uxíø="¨?Pԗ"7cl?ï¿bÚMß?‡×…hM²q?>1
		t?^èöé?~k'~¯?…ñ}Çóí?ï;zk\?™Òâkä|?n:#ùC"?aÂí¯Rx?˜qL?ê"¥?€T0É÷?ïæ]çíÃ?T˜R¦€?9"Îe¡?,hÕ~xCù?fo~³oý)?RÑâ<€8b4FGL J0611.6+2803?Ä´o
YD@Ð]{ZÀ9ïËñqÈÀ;Öè`·Ñ@õÒö\")@æuš¶Ð?čaûÁ?ƨºžÌßA@ÓrSÍÝ@ʺˆýj$¿à4³eó?Ö÷PÄh¥0¿ÚÞŝ®|*¿ä2>@­o¿è¬QéØ¿åd¹½üOqAGNbll3FGL J0611.7+2759GB6 J0611+2803?åÉ£XLF?ÀO Oá?"•¢£$?#!'Ö??Ԉ#_%54?À'ÈÞõ?ç¶@M§w–?ÁÝJûÍ?wùäKöÞ?'n[À™Ï˜?Ð3—Ó"ü÷?Á–Ž+}ç?éf¤?¬0ƒÒ€Þ?›^ÿÉÀ€?‡V"±¢?ÈPàl7|?©hڜj»?êÏڝl?"cr¿Â_?—U·tÌ?wÇþ7gË?ÃÝÊÔ¿¶?'þçÄaÔ-4FGL J0612.5-3138?îÍ4¸æ³JÀ5Œ
9>åïÀ9覨uÕoÀ<5Ûèɂ•@¸ïË)Š@îòžîm1?¶1Õ i"(?­õ}FLÒ?ñÒ±HL@³×1)Þ?Ӭȵæ×:¿äayÝf¢÷¿çéµ²¿èfu 3Ä¿æTg–NÝ¿Ø­>2­AGNfsrqPKS 0610-316?ïßú 8î?b}í3Š	R?>xúÀ.?3_ ×pH?l6øßGº$?aN'1f=?ïÈûÛE<;?}³®(»hà?3}Ú|ôg©?Q¨Y÷Š?zJ4µ'›¸?}C²Uæ"?ï*lçi?}ÛÆwá?iX9ïƒÀ?\S"ÎÎ?—‡{øe"{?zäï(³G÷?ï¨#Ò³U¡?h)'+l~b?^øä4Ðó?JèpÒá&?'îÐcýu?f%Œä÷4FGL J0612.5-3934¿³˜äÞì}ûÀ7ùrÿÑÜ×À:ÒȏPj|À<a3œå~t@蜞¶@M¹â}q?Ô%j­¥j?Ã÷‹<^«?ìJtÎ6/@ØCÊZ+Æ¿ã<~֟´f¿èâzžµÍ¿æ+@àðÆ&¿àó"aÌMÌ¿ïÿÃF1=¿åœúÂSw AGNbcuPMN J0612-3939?ïDÅÅٚ?Œ…Ïќëñ?P°ˆ'\Âk?GØx£T?˜½|^>?Œix^"p?ïk³óä¸?4N@ŠN?F‡)¯Dß?WÔÂŒ@?'èp4	Gÿ?ŽêÊp›?î¬ñõ,'â?‰³j
‹'‰?rýÐþõÄH?f'¶Ù7§?¢Ñ&^Én?‡¶ƒ¨]+¦?ï"Õݏ'¶?Dk$ûm?TÊkÆüu?I¿]{·ÄÍ?šXœ¡9\?~ F;9Ø4FGL J0612.8+4122¿âWÉ]#@%ÚËB‰ŒÀ7ïßlÁÕÀ;YKHÓ®h@wáú†n?ýQýýûC?" ç^Ñû?»Ù¥ß^[@ ¶ñýÞ½@¤e¹˜<¢¿¾+"˜†I0¿Ó™ä'¡¿Üýüdêæ=¿Þä[^Ëg¿ä	ó‡K¹¿æ°T%òAGNbll3FGL J0612.8+4122B3 0609+413?ï‡BI,?‡¯Çق¬¨?OXÐýP²?R­0Á¢?Œ9ëãùB?†È«$înj?ëyîÊ"ºf?Ä/|")Ñ?¨ÚÜviw
?·Ó$g,&â?·ÃsµqB?½¬Å¦¿[¯?íŸU²_Ã? Ò¡ÄxZ?Ÿq%Õ1äÜ?–z!9_u"?¦RïvÁ_?–LÑøhä?èûM?	2?­"âcõ´f?¥/RM(®?'6툈Å7?ÆÆ&7¹¯–?«D´÷Ær4FGL J0614.8+6136¿Û
(l¥÷@3Ùb¶®À: èj¸¿À<l³â;ë@35í!Öê@ž7€ŸÍ?Ë<b[ê·n?ÎWÜö:¯S?ûUÕ¤â¢ø@
8Xöh?ïˆ;¾/á¿Úf2CÊF¿éƒ<€8õj¿ç)L?Í¿ä됧'i¿å"ߨò}AGNbcuGB6 J0614+6139?ïqز"Œ?…îl0Ó?uõyáF<?r™ë–fs?ˆŽùÌ?«Žæ|°?ï"\'úÃk?š4ŠD^üå?jþŒ}Õ3
?zQM7Ñ?˜Tœ0ììN?–eã½)î
?íŒú¢žgç?–Ãñ×êt?"CáÒfŸ½?ˆqé5=þc?­dìæ1Å?G2Œÿô?ïylÉÍ?}"X]1?xÖSRbƒ­?a¤hÅÞÊÏ?–Û='-¾ó?|×ÌÞtH4FGL J0614.9+2426?Ìԗ±âæ•@§TßÔÀ:‡²Â_‹À;ó
8h&Z@´•‰¿‡?û´Õ)' ?Ø쒅(Ht?怸!D@X`~Åؽ?þ®ÓdìhÉ¿ïü0g¦ØF?ïüÕÞÄF?™óMa[¿Ö'×ÞxÆ»¿ìÛU%ÌB¿ïýCŠUAGNbcuGB6 J0614+2426?Ò[ž®¹Ò4?Á¢Ð
úÛ?¿ú;/òÞÄ?¶Õa𓙙?âÒéB¤»?ÄÚÔ6"?Í´Û ÇÒ¸?È(Én{—?Ƒ/óð~É?ƕp~'r(?âî}Ñë ?Ë>¸è?ݵÛÏóàd?±eœf?Æö·0
\–?§óùª¤·?ÖÎȘqQ?¯ Ē›ë?Ûnbè'AË?±ø²ÌúH†?¼ÊŸãkN½?«JG6±?Ý^õ"ê†?¶YkW'JÔ4FGL J0615.3-3117?íQ®žìó;À4ÛaE•5‡À:Uôÿý²À<hÏ(ǟf@ú¹žßZ@Ò[YÂéõ?½r¬Dìï?¦¦˜ZªEŽ?ç/œÛmy€@Á–vú]T?ïþ?üšE¿æ¡³^f½¤¿ã&Àþb¿áSÅDBO0¿ãÖàµwF¿Ýš_ý–™4AGNbll3FGL J0615.4-3116PKS 0613-312?ïá'àoç?ck‹[ÿ~t?6Z·ª­€?-OþµV[Ý?l-'ÈšÂb?b@ؔa¾0?ï±B0f?'*zڒVÒ?46Ûæû'Ô?D¾¢âm?ƒø"®£¤?¬¾Fûœ§?ï]6­K?UCĉA?ddž´&Ù?Rþ$
³ÙK?š[hSÚѤ?€¯¨Ä;'?ï(ÆÂç5æ?{-¨ÿìZ?h‡i[.?RŠMP.÷¦?—Ö:q-à	?{çr±>4FGL J0616.1-1732?Ø0eäÀ/j;Ýü À;~ì\µ½À< Òc傦@!÷ŽsuÃ|?öښéœ?åö\å®›?Ù¨Ã"ð?÷†D·%?þўEzÞn¿ïþ'!€-b?ïôJõǗÚ?Ñú±AV¥¿Ø2ÒûÄ¿ÛÓmE'ÒW¿Ü  0÷ïAGNbll1RXS J061609.5-173313?ï=
÷P'ñ?›C«m¥Ví?]Ú÷ëHÃ?[pɖ¥²?–€ñ—99
?š¦c䘪?î۔˜µê?©EU\ד?`÷íQI‰§?qά»?¡7@`Ë?©Ncð
?ìäÓ÷‰ì÷?Ÿ>Éòþ²?ŒáÓy—?"ñ+Ïw?µ=%ԐM?›N릘"?ì['ÿ2A?¥|8?_`?XùÝ
¿H?_!Ä'mT?¼ÀùȘ?¤ý#n¨)4FGL J0616.7-1049?ÛeÑ£À)"Í[h£À:N.a<[À;¢ûú·Á£@G˯ÁN>@ãÖáù"¼?ÐÄR1ž‰?Ù¦žD¤Ù@ñ©áyñ@—rÄÔ?ïÿéà
v¿è@‡å</[¿ìcMâáâ¿èá}ÿ	_û¿ïÿÿ" 5•?ïù*ù¨ÍêAGNbcuPMN J0616-1040?p|99?¦ÿ6Ôï-?ˆ´ÆS=ý?üÍÍ)?Ÿ'ÆÚt?¢}á·í¶?çµcÚ§?ËÒÒ<¼?´ú:)c?¾LGÊ°7Â?Æ®…pV5?ÆÌ@ö+?áß>máÔ?¯]Õÿ:¸?¼Ÿºô†?òæ²p6?Õ"g·?«WÑýEïÏ?â;`º(Ç?´C¶ô£çá?´ìL*kÝ?žÿe±çlp?ÖN+­]?³)Là¶4FGL J0616.9+4340?íuôØüÓG@)<ù;À oÀ;ÚÂXՄÀ<À­°i@"—¤}£Cç?ù¼'«A?Ø	zg¥*Ç?¼O ÒÀ?éÙ? ý&?÷Š¿Ì‰0¿ä¿@OÁß?ï«ù4㍿ٸ)|¦Ù¿Ý&c–þ4?"™húÈç¿ÜºÉ?$AGNbcuGB6 J0617+4340?ï¿Á¿Î?¢!‰™v<?E¹¸³û> ?FŸ_i«h?Z:feø?¡ÜMUåžÊ?éWÁû…?Ëò}Ñ2'*?vžlË%w?‰qãVHn?Êù­•C˜Á?˧ž>¼<€?ìë"Ö¯¾Ñ?›¨r˜ö¡?}"").±Ÿ?qu"ÖèöÈ?¶Êï_?šK#­? ¥?ëÈ6Š%ïM?¦··ŠÈ_?pAuâ½Yœ?o›-o"?À](RX?¦åºÎÃAÍ4FGL J0617.2+5701?î*
ÍäNõ@2ëáe
FÀ9I"žˆÀ<(ØåßÃJ@‹AÑ܁ @a´5&Rz?¦DpÈ??§_™m¤É#@"'Æ@
Ð-µý­¿Ñ£ˆ{>1¿áZºÌH¦¿âA¬=
LŠ¿Ü"ëø>ø¿åø| µ¿ã^'/éAGNbll3FGL J0617.2+570187GB 061258.1+570222?ïë…û8?Wú½HN'?4óyì$)ö?,J#àºúë?aەÁCeƒ?VH/Ôd?ï…'9æøû?'5½{j*¹?T?AÁ±ö©?g.I˜T?Œ.IN'7?6£L¿)þ?ïR‰{?xҘ%é?g‹&]½€?]õÀ	ÅyË?'Ýœš£?v®Œސ?ïñ*«	ù?rW€HÏÅ?sê]Ùl?a}H¨–?Îµ&·•7?iíDú×] 4FGL J0617.7-1715?ÐíÊ›¢¼À.!6ŎêêÀ9"#rËÏwÀ;Û¢4rÎT@‹-á
¡?üœ¡ž¥r?¶¢?/•ÄÎ?¼ÜÎ!¶‰@¹ÍÄC'O@v]ÃՂS?ïã3@Ÿ-¿àÅã~ê읿ÝÈ輗u}¿ÖÞ$Þ[À¿ÜàA>
ׯ¿ç=ý¼ƒÔAGNbll3FGL J0617.6-1717IVS B0615-172?ï×+›¬˜?'AT"-§?pœNöâ¯?evëmì?›>Ït?ƗNψ?î÷EqD½?œ#ŽZƒÒÈ?im¥µØfw?sÊÙMÿØ?é%ü[¯?™ê'Ó
€?íõfaM?ßԛ CÙ?‹i¢Ýÿ…€?€­ØR"?´ƒ tê?™a$ä̽?é?°´
<Ã?¡ê¤µ[¦?'s¥±?Œ‡?uœ̘¼ü?ÈÒÈy¯b?¡íŽW®Ÿj4FGL J0618.1-2428?ê"#ÝøÀ1՟+©ÑöÀ:Žîr9€À<Q·åž@ñü"up@ÅsS6?ÊvófêoË?Ê\o—'ƒP?ûëlË@5'éþâ¿çzŠªéM6¿Á™Ãàêç¿åÈÜä.¿ã"I,«¿íÁÍÊùö¿ï‹›ÿûMiAGNfsrq3FGL J0618.2-2429PMN J0618-2426?èü𞒍'?¶­NuüJi?¥döÝðrN?Ÿ+ÐÂÊÚ?ƲÿÎ9­d?³ë³Ò«e§?ÈåDl?¡OWȪ?tû3¾-M?ƒr«†šŽ?¢Ö\ùæ©?âb»Q?ë¤ødÍÍ?¢Ví •?¢UËñօ?R D
õ?¹­Vá
(½?›u7ÿV"?ìHcY.Ç?–O Kí·?™m3ÁàìŠ?ƒ÷fs‡Ë?·a˜GfNš?"͈¼ŠMÐ4FGL J0618.9-1138?ï»Ê0@ªÀ(Ӝ"öœªÀ:%'ºZ'À;±B¾ÁqO@¸w¿T>F@	1)Ì?Ïåwh—C(?ӊ©|:¹@W
"˜±<@
¯î~Î<¿ÞUµßJ}Ó¿Ù@½!Þø¿åÒ!ÀšŠ¿ëò9Wÿ›¿âÔrþ¥7¿ïÿ­AGNbcu3FGL J0618.9-1138TXS 0616-116?ïìz{$ò?Š£-º½Öa?VÈ#°ù€?Q³¼MŽºq?‰«àüÀ¤š?‰«]ˆà,?îœ[¾¹ª?¦É™eÞ¸?s93¤Óo?‹ZØ'äí?£Ó!MðÄÖ?¥ÚÃVÍ?èWÀ`X¸‹?¬–D^9Fô?¦''øóZ?'Ý"'ŸŽ?Èüš`GJ?©ÇïÜE?ëèiC´©3?žä)©x{?|ž=¦ñ?iT"®zV?¾û›þ€T¨?žQ¢ÀÁ7n4FGL J0620.3+3804?ì¾Ïµ¤+@%|L7æ÷À:5ÉæhÀ;™4A@3X¡¬¸…@#ŒÚnuÿ?ÎP¹ŠÖ³?'£7'3 –?Ñî¼t@`­Eîé?ì8npöã!?Û{ļ²ù<¿éÓ¯ºmO¿æ(ýð[GN¿äêîU³¼¿ïÿöZdÐdAGNbcuGB6 J0620+3806?ã¦Ì»òÙ?Å90=¼?¡~â…ÜRt?›b-¿°1?ւ‹w̏ÿ?ÄýöŒZ?â&»aœ"?ÐQÅö<uo?Ÿ–ì÷"'A?°ÊYÄ¢?ÚC¹Ã"f?Ð^#™D?Ùðñ!o?±†·°¢a"?´/	ßѵM?™Áîéfç2?à¦3N<Ë?±(˜B¾‹ó?ÔÑÓºæïj?²÷2tÞÁ»?žÈŠCÞBx?rªHø@š?ä ÑÐm–8?³ ið Ø4FGL J0620.5-2512?î}2•Ôh"À1™ºç£À9¬6KìgÀ;å &5@añµaÌ@]d_%)…?·ÈG¾àù?Ï°%1½½@WƒPù@KF?jú?·J@€x¶J¿ã*óÿ@½_¿èYö|É¿èæ	ITݨ¿ïÿé{2¦¿ÓÀâÞ±ü'AGNbcuPKS 0618-252?ï¢ÍR°;?§'­@Bj"?ƒ[ª/ƒ"?¤ÇÙÚ¿¤?`é?P'·†?v¶ž	ZŒ?ïy½"Nµ¦?"=YÒ¯Êl?`Ü|Æ®¯É?t`ûWM?Y˜:¦êi?«>
™n?ìBȸ¦¤X?¥_æz¡Ï?«\ŽÖlè?š"dŸĖ?°;rϔi,?™¸†[6"?÷ËT?ˆû'7‰?‡w"|ø??sVñSrR? ²¢+¡?†
g%ƒ®M4FGL J0620.7+2643¿í¥ÄF˜–@¯^AÔ¶¦À:¡…}'ãÀ<E-5Ã0l@#XÅq8Ò?ø‰{>d¿?ÀÜ gS¡=?¯pÐDÅ?ñ&'+½óì@<HQRƒ¿ïø½Ÿ¤v¿î¿ >ybm?ïÿ!ž5_³?xõá)a^{¿à
Ç9G¿œô"'|êAGNbcu3FGL J0620.4+2644RX J0620.6+2644?î>°;z'?«ÜX€K"?Byi-ž9?CÙèg×^‰?«ÖÏ£ }?«²l[îÐ0?åÛÄB©ñ?ÊWaÅ&R?nGÞ{á‰O?ZÌJuˆ?Չ¸º'é
?Ê
BRÌÚ?è÷Lö
62?§ÿ´ÌÆô?'þ|AÞ֞?oM-SÅéÝ?Êòäc¹9Ì?§j™)LŽÔ?êŒWܾo"?©‰eR½?m¶ó¥{R?m˜X»wÂÕ?ÅWľpT¦?©jo9ñ‹%4FGL J0621.2-4648¿îis¿}fÀ8]æ?À:×Fšï/À<{«?´Jö@€Ñ¯	ÃM@Ò>ƒÉM¼?Êõ°kϲ?ÀôºQ Ä?ïü"à՘M@Éf'0CÀ?ïԉ>؂ã¿å©é]|2¿ç)y
­Øì¿ë);b¬'¿ïÿ¾ú¿±€
A/šAGNbcuIVS B0619-468?ïÎ8š¨w—?r-&ï™Åc?H MÊùdb?DsnÎ%,Õ?uߨòe\?q,®0ÿæ?íù÷èñÇ?­ˆóTl?€€Žƒæ$8?"CºZÑ#?¬@]Ïôº"?©ŸºÛ›¨?í͸кJ‰?'_Úº?ƒ$
†àª?sW¬Öf?®=)ðùŸW?A6ëdµ¨?íx5ߚ£?'cEµÏzÍ?DŠ<éf?yÃ=`)Á?°-.t&X?Žš¤/Œóf4FGL J0621.2-2213¿éãÀ¢-MÀ0LY§;BÌÀ:¸
!Áñ§À<vžy_g@"SCôÌp@b5deÛ&?Í/ÉÜ­j‡?Ï'쮤@=–é»ðÜ@Æi'wâ?íÌÙ,V  ¿äˍ Îí¿ã§".οâ.0y²É¿í*áã¿ïº«ÍxÄ7AGNbcuPMN J0621-2213?ìÍ
>ÕÛ?©Ñåcœ?ƒw©Fd?z¥È½iùÞ?·(¶Ôˆ\?¨(O4±F?î¾	c~»Y?¢ú‹Ÿ_\?v34T²r?ŒÝÏU %@?¡YG	´0?Ò÷?KjX?íÐ9++™ï?"úôÅáÁ?ÈÓý¡â'?'î΍¿×†?ª˜NuoÒ?Ž1VÅ×1?í¥jÚ©?¤¡œ±f?ŠhÝ`¼ÂÝ?r£sf[D?³Õ¸ýº\?S"Y i·4FGL J0621.7-3411¿ï°,ù2[rÀ4"D€bïÀ;ö¤À<‹S+ ?;@ L'Þœ?þZ˜⚔?ЙÇ|Uæç?Äx†$?òbI$.?ÿ‰®ww/â¿àÈA§õÓ¿î1­ÂEŠN?¹ú[?/¯Š¿Ýkq}›·+¿ãQf™'
¿âõÚã1AGNbll1RXS J062150.0-341140?ïÉ‹R?"Ùﲔ‹¸?RKK"aêñ?I2QK®†È?œ*ŠHw#?"hbâû€,?îÄêXîÿ?£1÷áÌ¿>?cî¦ñßÅ`?sÊ8Ùb= ?¢rukS²?¢%6Ÿíà<?îŽÀ"]˜?"`5u?q¯Uã¡I'?^÷p¬º†I?­¡)AeýA?ŽGƒ9߬.?êîñø?m7? ÷óɧ32?r*t²ªë?cÑdŽŒÀ?òçÛ\µÌ? èŸƒŠ'4FGL J0621.8+1746?á¢gÆ/F6?ûyŒ³Ø	AÀ:¬¬ÊÎÅËÀ<Û£)eT@!å°²9ùv?ýË?.9?Ìa2µ^ñþ?­Í bSºÆ?áxg_µ0@<¹y]å?¶ÁŒ@¯aq¿ïÿ…ãp?ïáeáhö¿áQÛm¿ÐÄށU*)¿Ù\+d‡¾üAGNbllRX J0621.7+1747?á·¿w(?Å rbD‰?\îçÀ~?Q*Âú''?Üu½‹™Qž?Řдä£Â?ßwÕs|õ?ÒIúý@Æ?g¬C£C!‹?€X¿B?à,ižBQ?Ò?ÏT0E?æäÀÌ´Â_?¬O…cэ?Šdâ6t1¸?wS'Z
?ÑcWTâÙµ?«9ë·×-ù?ìŒô
,ç?¤²ݵ£?QÙFL3·?P{©´Ý©/?¿@ú•gò?¤¨´köpÓ4FGL J0622.3-2605?ÎÐ53_öÀ1ŽPÅë1<À8w¬-ðÔÀ;¢ªùš‹@ûNuÙËä?ý÷dñ`¯?¢¡È€üƒŽ?
YJI$a?úbxÐÌ5Î@8xé@¿á䥜[d¿ØqCå+B¿Þåe_€C1¿ÝÔY¨‡s¿ÚðÁ^.´s¿Þìþ¢˜œAGNbll3FGL J0622.4-2606PMN J0622-2605?ïñ!cø ?S°ñ`¯?"7ï¹þ?.:±a<ó?[ôÎÊ	?R'>Ķl¦?ïن~…)û?v`§ÇFøN?#ÝӌGօ?=Ò¨EÖ|€?rÒ!Äz?u¼Á›Ö¢?î¦
ŒË?"&èñ4kk?rK®Œ(.‹?p"'ÕjÊ?£TÉU¹}~?'H|Á~ù?ïɨçjçò?cøûËZl?3iÔî'1É?$/æ‹dà¢?yôîû£ä4?c‡®"04FGL J0622.4-6433¿ãp»Ô×ÞÀ;bÎ-±êÀ:»ƒÑÀ<W0º²îÕ@zô»Ô,@¢¶®}Vm?ŝßN"¿°ÊkÞöE?å"Èy€õ^@'~øƒ‰ã¿å@¯½ÈM¿æäÚ_²m%¿îA¨v¬.È¿ÒÊrŸ¯³6¿ÐgÕÒ/¿ïýßßy!ÕAGNfsrqRX J062308.0-643619?å©×?'(uM*?eú"ŒÀ‹h?d/£§:?†!cegŒ?'V±õpÎ?ï@'ÆòŸ?©4¡™°?WßNè—ä*?q>5'׍?œyø¸˜-é?¨º?¤I™¡?ì¥Èè±<J?ž+ÿ¦ÅÒh?'y …-È?u"Š]ו?¸'©†ewù?¹³·	Ž?ï¦ùšµp
?yR6Ÿ?SîƒÊÆø?V bEñ°?ƒÃÈÙcÄ*?x
íÌT4FGL J0622.7-4141¿Ð…3ÇløÀ6¸¼M"ÉÀ;Ć­-ËÀ<ØmSÀqu@œêxÚ1d?ÿ¤2‹m‡?ÈeŸA#`Ø?ÛKkä)µ±@g ã¥Vf@ãNòï¿ïÿûÎBÓ?ïÿÌÐJ†¿ÝÌË_ºOÈ¿âqß«Ì¢¿ëäò}¶d+¿ïÿå]½JyAGNbcu3FGL J0623.1-4143SUMSS J062242-414357?ç풅½3"?ÀsƒÐ-oƒ?Êg3Hu]?¿ƒ9pîï?§Š
'X´n? î5$gME?êÄDˆ@?¾~ 6<\"?³Þ‹€™%¹?¶ÞcädñÖ?»"R[$Ú9?²^X"vò'?á¶t»ÄÒ?´º¤?Ëï?Ñî}¦P†;?³2׶À?ÅI4Toà>?¤šr1
§°?éá]Ò§Äþ?¢Ö¨Ù©M?»GzÝþj?œïÅ ÃEF?µ­—Pãٞ?—½3e#ï4FGL J0622.9+3326¿ä¦Á}¨@"MŸ±áŽüÀ8k"ÌÐÿÀ;fr° Ĝ@VfXN ¢@D:Âs­? §?ä5bý?´8p)³®@KïIÏVë@azXᘌ¿ÑI
`EË¿Úölmçd(¿äÿ­õœ¿áWÂ~ë'¿éB=äg¿ã¶ô›»³AGNBCU3FGL J0622.9+3326B2 0619+33?î%¥].DÅ?–_I?Zs)ÞºüÍ?Q^®œ‡K?¬ÒÞ%ÛÌ?j›ul_?\óC·?›ZV}rSO?G¦"Cì"³?eH9³fÂÅ?_@~ðPN?š²ßv?îd®'{?–Ï0!,?†ç-p‹í?'®¤¶¡',?£û/£¥@?'syC¢Öä?ïöe¹–t¯?GÜ&>P—?Øj+¦·?FÀԁ ?RuɁ½ü??G‡¢°´æé4FGL J0623.0-3010?ã÷ԑ"ÛÀ2ëèPïÝÀ:Žf5¾þ®À<WoŠÑ€@sªZ1#ä@üCbU_®?Çy-¾T9?È´͆†?ÿ4i^hk#@	—49˜}¿ï©\ºëù¹?ïþ•œ´×
¿çýŠ¥
$¿æÜþ]¾w¿ë>ÝöÀ¼¿ïÿå(
eCAGNbcuPMN J0623-3010?ïÊòeX?qÐÁXº¾ˆ?`öx°?[ìòiÿr°?rx"Jä1?lFÙLÝË
?ï¾1yÎ+?'vi±
§t?:ÀÇ÷‰ÁJ?Q‹´?;6÷ Mí?w?vüè?îT}1ÕX?'ÞÕ?ƒñl¹?vÁ6ö(ua?¥øÑÝ|?ŽQ2»ö;?ï|nֆŠ3?r#¸M
z?ow^já¥?Z>ìlyû)?‰rÞB»?o‡
.Æ4FGL J0623.2+3044?ï`ÕðYfE@ ¨½#žÀ9Ù©-‹TÀ<E¢Ë@ ¾!Š?üS€*\ÊÜ?Àµs>æð?Ä=ʗ"Z@'üÕ©@&ïjÜlÓ¿âDrØ
¿æBw©"É(¿àø]©ÿBk¿Îêq"'¿Ý`QyoW§¿ç®Žd•AGNbll3FGL J0623.3+3043GB6 J0623+3045?ïãGùH—?'ûÆî«U]?dêeъ?`,
|[Ò1?™æE5RÕ?'ëת?èi8þÎ>?ÆڌpœGo?p¯‡=Z?'ξ¢zÞ]?Í՟Ì5ó?ƍâÙ'Vó?ëÿ¶'~5?¢)«!?…ú)èÏ0?vYÛÆul3?½C-ú.;? Ìûœc@¯?ìVÅ?š—-ÆÏÉÝ?"÷º§€²v?ra,"'ÂA?¼¦X'w?šÊJÓ5í4FGL J0623.7-3348¿íÈô&Ç®ÅÀ4[À6ãÀ9ìuk¼ç|À< 9€
@ Z¬Hóº@bê¾O[ˆ?¶Ô? Á†?ÆÌV»£…@ºk
F@ëc`w?ïeáÜ(Š¿Öæ€',À¿ääµ Þ¿ã²æ!1¨ï¿ë"Ÿ»Ì¿ïù)ÍAGNbcuPMN J0623-3350?ï§ÅÖU+o?yªÜ2BF?t'HÛH1"?p¡¿	pó[?wŠËú"Q?l'€Òð"?ïÄÄskµ¾?~ºnLc}è?=+Ô5Ñ?X Aki8,?{Í™7Ýy?}}>֌(?í;f
I3½?ž';CÄ?£è}—¡3?"ô*~á
?©@¶ÝÕ"ñ?'Œu×½û?ïGþã#?}Ú'Ò?d¢ôE¸µ€?RŒÐà%F­?"kÅäu®?{kÃ¥ñ94FGL J0623.9-5259¿æ¬ïH'ƒÀ9[ѼrâÀ:è	¬Q,BÀ<£O•i‰1@yfÞ±PÅ@Á¶ža?Àd鎤s¿ ©Ü1ï'H?ãæ¹Ù«@K^ù	¿ê''Ò¬á?…pU0ð¿ä&½2%¿äO%‡N"¿Ò3f~¿á> AiõAGNbllMS 06225-5256?ïS'Ç™T€?ŠaÝÐ/øˆ?V†éµ²4`?IõŒJzßü?"%8qzL¾?‰¼³šY;?ï] _!À?'X4½èŒ??%F³]'?S¤ó^N?"Ï]Þ­1Õ?'æiòA?íëð6'9?£6ïk¢?z.6ãyá?góý¡oö?­þÐýB?Žß}kGãù?î¯UsÔ
?†Á|™I?c~ò-rH?VÔ¯%t°?£ÙŸè?†åfY=)4FGL J0624.2-2943?ÓÁyñnÔÀ2ƒ`¦3À;-Á>#Q>À<šnkîe¤@ g
Tý2p@2fâ(r?Æÿù_|è3?'îƒx<t?¸paö"@íW<ý·P¿Ô5k×ÌÛ¿ïÕrùà0?ëFúû´@å¿ãÚ­Ëų¿ê&ÏAò×?ÌJry\ãAGNbcu1RXS J062422.3-294449?.4®?¡¯äwRüA?gB"Ö®­÷?cd')˜ù?¤3ßTú5?¡ê/:íÁ?ïU®ô
R?•Op< ¥¥?OjX0:?'?\Ü<θÁ¤?"Nλ\ƒÚ?"'A«¸ø?í©'–< ?•1x˜¨ÍW?ÄՏUF?{"Ô¸ãr¹?°z؜4¦A?'=—¤ژ?î7©½ `?"Ü ؄m?en*ª›–×?b¸0cuZl?«8¢¹|@?"ƒ¼HSèú4FGL J0625.3+4439?ﹺDm¡@,Èdìé¢ÆÀ9p-ô/fÀ<-ëÎð"{@+'þKË@j0¥º9L?®Š°av|?©|ýÇ%C?úÔ:I§é¾@
8
û1¿Þi"$a¿ÛQìüíüÈ¿áÖ¸ÞÙ>Ë¿á&ƒÝo²@¿â¿Ð/WÜ`¿ãºû~ÿ—AGNbll3FGL J0625.2+4440GB6 J0625+4440?ï݄ý°â"?hz"ëÿ~Þ?7&ùùþ?-E_ˆ†t¹?o–#úü¡?g—§Ð>`§?ïn9Ve	?Šbо?KŒú"¼N´?_ªå¦Kµ?†ë¢øî?ˆßcI‰
8?ï&®R\?€ûª¨Öª?jºAƒ":?UÆVޏ?—çB3c÷?~zéÒ¦G'?ïYÎ_8<?wB\Ž˜W?tïà:›+?]{ÖM¾?€pAÛ£^?t6ÇbP(4FGL J0625.8-5441?ì¶8:ÈÀ9o¿aª?À:5C•%À<VH˜F@Úäå@o–@HÅl?¿o"͊aî?¶šÇ—æd?óƒ
€òç@	¡hðÚH?Ë&`¼Ù9ÿæk%^¿ê«ᚺ+¿ãu"Ód—¿ïþŒÍÙ<G¿ïô€d{AGNfsrq3FGL J0626.0-5436PMN J0625-5438?ïó{ÛK®à?U×F@50?Cq'·	Å?A—«šÜû?NŸk;vp?NVXµy7ÿ?ï mTŸ¸?<:hO€'?Gۚbßh?ZymÈ©?Šº+·$+?‹lÑ'r?ïFi†þ|a?{¥À2g?kà
áσp?[âŸ!äç?"¶Ícöƒ{?y'+¡í×(?ï|$ïlü?t	³Àx?x|½"-§?fŠvH.†`?"ñÅöæÃ?l±¶\"eÎ4FGL J0626.4-4259?@1skÀ6qgÛ±lÀ:gØp¤®À<rZؓªl@ =é[;e?ùXñ°C?ÑIÓގì?ÊGçµ±RH@'í]f¤@-æ–Íar?èM!*È+¿ä'%ߍš¿áŠJ;tÈ¿Òu.`µ*¿Ü4%áæåR¿éäóiï‡ãAGNbll3FGL J0626.6-42592MASS J06263670-4258059?ïÓ|YXb˜?q,7ÕcR¤?;ò`q@W?5ç˜g<E?t'­Lº®?pWE͉²?ï·.Kéh÷?^´"¼i?71߀–Žu?VËÛu«"®?zÞ	¡
Ë?€wgr_p‡?î<•ùÊÏ?"³ÜÙºnD?u¿¨m‰šJ?jەZO@0?«äA'²É?'n#µ€©;?ï7¢–§?yyûßÐáÍ?I®¢ÜÒàs?>s×p	ë?˜>8%Å^?yÕ#ë94FGL J0626.4-1712?춁	»ü¬À*FhEZ}À:¹%8ž¬ÿÀ</½ÿªo«@<ä1˜Ss@<à[?Â¥ýÖ.
¿¡K×ÄÍyñ?àwU6":@bÀõ(5©¿Â$ޜ-Ä¿æb­¿keT¿ê'v¹Ã?²Ò<ççÛ¿ç+Zâ#Ì
¿áã+~3ÆAGNbll2MASS J06262650-1710467?»0*?œÓöQ"±?pzî>xä;?t¦ÿœn8?¢fæ†íàÐ?›mÎ*þº?ï7
Ø*›_?¡È½F9Î?AGkµNâå?P=N J?˜"iý?¡°õ½?[ž?ì"Á…²u? ßc(?'gر#¥?s7æÁ¯?¹äð¼Gè?ŸïHlƒ0?íá5àâýa?—8¦8]?xà
æļ?py¡Öº~?®Ð "÷¦e?–J¿®V<T4FGL J0627.0-3529¿–ËÆts8À3ø2¹¯æÀ8êe˜ºÀ;ÚꃖøÕ@è7cnU?þM€†£Ð?¥I['Ý?'AÒiCæ?ìf¡t¯T@– 5T –¿¦áÃ\"31¿ßZžœ¿Ç¿à[Õì¿×Â"µí¿àŠEžoÂ0¿àæÂÂ1é1AGNrdg3FGL J0627.0-3529PKS 0625-35?œ²Ï•?€\›%œW?JÑðpMN?AO-»³Ì'?ŠfyÌGF?hw˜öÞü?ï²e~&…?…ªˆs?>Ì7rOr™?TM$ZÒڙ?'p>ºÌ=?"¬^?îZ·œh*?–°S‰?{m2Y=õ?xå >'R÷?¦ü¦ßîU ?"A¦	Q5p?îÎ¥7ýü?†Øå¯DS?r2´'@A?^ó•ï'ã? Å†)«E?"¯xðùÈ4FGL J0628.6+6900?ÔK/.Òâw@75`A‰7LÀ:¶çºŽÜ§À<¯Tæb4@°´k½@j= ÿ:?ÀF¨0
_?¥0¼ê½µ?åAa)ÃÂ?üPåüéö¿Ç?›5ûåi¿ßN€2ÀG¿Ýߋ€Ò"w¿æîâ q¿àáÕ<ÝÖà¿å¢zH›zDAGNbcu3FGL J0630.3+6906GB6 J0629+6900?îªÂ
ÇI?"ñý ž/Ý?xi¼kî™?m€nÝåá?¢\6§Æ
¡?"[Ú¶ª?îɑÁ@O(?™©V*¹?iÜG~"¨?qèꜸƒ.?¡Étä#?—¨»25Û@?퇮w	i?"šÂ§ª¼?‹Z1;T?}Þ:¸™<M?°WLAŒ*"?ZRzŽW?íèí`°??Š€óUÙòh?þ©ü"Rn?záü8¶?¨ñÕ[R½?ˆEߢ&æ¢4FGL J0628.8-6250¿äfPxWCxÀ:vø½ì_9À9—Ú\ØHÀ<]õ£…«¦@Ûwy´!@ä̂úñ£?²ñLˆï¨D?¸¨xY­ñ?@GË $b¶@i}G(‰¿Ü¹­6/¿ã/¸ToÃÝ¿àÜßõÉp¿ãòžþˆ[¯¿â.•ßе¿ïÿîͨ"ßAGNbll3FGL J0629.0-6248PKS 0628-627?ïػѾ'ü?jT?¢˜?@Œ‰jt?8/؊ÞT?q…ýÀq?hðüCö?ï"X]4?‰/ÓËè?DãFy‰ß?WöǏÙÂô?‰›´Ra‡ª?‡é:‰Ü?ï/¡üb²¤?€¦±æχþ?p©æìç'Æ?n
P7	c0?•áF¸oÇ?zé?¿{ñR?ïY*lõ€?x÷M\X¿?nyÏ6!ûà?WŠý¥ýö®?'€Ë{?vt"±½Ö4FGL J0629.3-1959¿è "ôûÀ+U›=ÈKÀ8¦$'–GÖÀ;ŸñvÐ@ö@í®Š)@/L{ٕ2?¤þ€_G‰?²{婒‹@7b|×Â@¡ù5‹}!?îÿ5Ÿôým¿à;Ø»¿ã죗I]A¿âYÿ ^¯¹¿å•[|'˜Ë¿èK×nç>hAGNbll3FGL J0629.4-1959PKS 0627-199?ïÈ@ =k?n,–ŽÑ?/M…Þ!Øè?&'jÀ`Äd?zåC²‡¼?n"ILúQÁ?ïÞ¯Ààˆ?tÅ3/RÒ?#¦ŽO`?9åj=mû?p
ë}Ãò?tÑ¤¹?ï(#Æöû?ß
aç}?r*¤íÌÑ?eÓäKþ¥?™X0Ý孄?€(F:ò?ïØþT⃅?`Ö~£?2lCYŽäÇ?%ös€`"?rZY%Oœ?_FZhh4FGL J0629.6+2435?ïâŒxã…e@ë—¦zSÀ:w,50"À<6¯A@ ,IõÂdi?þ§,yێ1?ÆÎ'€L–‡?ÊÜ >ú;Æ@Ó#þâÊ@`KZS3¿ìõcߣi&?ïû0Ãj¦?°\ڗe¸¿Ü¨
»)Œ@¿å­Œ?¾ÜÊ¿åÁЄè1­AGNbcuGB6 J0629+2437?íØþ¾ù†¼?ª0#`a_?rBÍä?nTAÍT_Ü?°x¶_I?©ðÆYØ?éçx(µB?Æ	óY–?vʊ"Ùƒ©?ö@ Ä³?Ç«Ë^Ø?Å}5¡c³à?êÃ(–ÖVã?¦¨*¶l-?Ãk­wS+?~¡Eðú?Â÷&éÏ/=?¤k¯ÿfé?í¦Éhê0H?ùæÛ`ñ?‹'Xq|5Ã?x˵,øKå?®²ÓTýî?ð É5ÞW4FGL J0630.2+3228?èTÊZÒc@$4D‡BÀ;Mä·¥[À<}Pǘ°@ ÿ€Êì?ÿ°g܈+³?ÏMyÛc='?¶"¾ì†?é\>ŸÍæ@Xg‰Q"¿âÄõ"+y?î°LÎå«Á?æÿN)X¾Þ¿èY¹Å¿à9™m$?—àèžË˜ÖAGNbcuNVSS J063010+322608?è¯ú/¡'?ÄW™TÄç'?jì,aâ?cC-z€?ÌؐÊ&0?ÄK—àò[?êE9)áG?ÅBëÔI~E?s>ê²´k?†Ò˜("S?ÆQ$5ǵC?Äð·('™Y?꥗<ßKÆ?¦f5&©¤x?‹<Aʵx?x˜š2I?õâÈf%'?¥E×C€d?íåi*cÃÚ?™ª|_¾"?s:Eʓ?sÅ'­V?¯B*±
oÞ?™9/*Âw4FGL J0630.9-2406?ïS5b&‹À-ý˜ZÕ8¬À7Å™m#ðÀ;'>[…b@â³¹€iÈ?úw¥ôïp?›h´§ð}	?·³ìŸ@©"þ×áÔ@²¤­sì? Õú¿É¾¹ä'¼0¿Øtߚ¯Ä¿×{Ì¿‹Æ¿Û½ûx±Â…¿â™
'¡/AGNbll3FGL J0630.9-2406TXS 0628-240?ïìÊþ&Uï?\fFzëê?9¼Üp
t+?>àl%šf?_ú̗PÁc?X×
ÿ[(R?ï?â"^óÐ?¦'AƤ%?kÐÑ›ó?áª7qö?"‰"r‰2d? #JV3þ?ìþTm™c[?¤åe…³—?—»◯?'Ü'àÿ?²Ûd<?E?¡ÃÙÁć?ìª'Èͦ‹?¦ƒçW´?}ٔF¶?pÞü7,Ë[?¸Ñ(u2Ju?¦A=&^RŸ4FGL J0631.1+2020¿ãäр26Ö@gŒSâÖÀ9kÛq«>À;—Ìe÷@@غÿñ@á">¿?Áݚzj)j?Êâë݉2™@'%ùŽÌ·@ð{Dü¿é7FBÐ_¿Íñ<†C&¿á§˜úà¿åàZéZ¢
¿çÀØ!ê‹z¿ïü-ãhÅAGNbcu3FGL J0631.2+2019TXS 0628+203?íK͟_jq?¬¡ŸŒ'+Î?tòBÅãöV?rõC*xÚ?´Rnئm?¬X¡~¦.??íŸ^ýw?´µë uæÅ?bÒv*9úù?vâʽ!Vú?¶ðïS¶Dq?´XâáYì¡?éij¹_£?©{èNÝÎ?¡뛊'˜? ‡~!í?Ä©ºJ7÷Œ?¦Ι'2?í~é'Y?"'M¯¾‰Þ?z €ÔŸËñ?a6ïǟÖÞ?µšª	ðx?"¼±ºyñ4FGL J0632.0-1032?î³ݦ0MÀ"ÞÁÁÖÐÀ9¢sۍZÀ;¶^	}@‹0k,ɸ@æ*C hÁ?¿Ø×á—?¼ô
ÔDe`?ú̺=~Ð?ùqï-Iå¿áí¾´Ü?¿áđ?h¿âJ/-êôÖ¿çaZž:Ø¿ì‰OŸz"¿ÚCTþßïiAGNbcuTXS 0629-105?ÓPŸ)q?À[-©!ë?—|Žf³27?2‡1@?å›ËøFeµ?À'"Ž^/2?܂=R•P´?Í8™—E`®?©ôÞêÂ=?¬Ê±3¼k?à"h+ƒ?Í=4ˆ£ª<?â澆{3?­€°Z}†?µh¾zƱ?™ÿâpЋ?ÔØSTX<?«SC9O^g?âXºo×ø?°D~˜¯{ª?¹Û»Àvó?¡ßÞñä?ÔÙ›ÉÔ?®czš/4FGL J0633.4-2222?×OÂ]昮À+‰
Z[–)À:.MeÀ;ó£BÇ‰@Sϊí.@##—´½?ÁhÞ»·§?Ҋ¸?Ìô@"]Ä×5@f§€âéo¿åÛ1´­ò¿Ù§MKã-a¿æE'`À48¿êðÚ'ÿ"Š¿êŽ€á¼Èô¿ïÿ[ËñrAGNfsrqPMN J0633-2223?ïj-Ã^¡?z=¥G÷?vlúFÅþ?qÙB¬;`?Š>Õ?‰$†½ŽK"?ï²mì{k ?Š¶6{v"?Cˆ@ëÕ
?]}äjã­?',Ògç™?‰±§P²v?鱅¡³3°?©ÍÙHÄ ý?²SN'=ì?n±'uî›?À`Ò'H?¢èÙHý?ïC«q€ÿ ?|ß#T£šÈ?`—"¡Ùú?Nn¸rcº?•‰ÞÝKн?{{Õ1 Þë4FGL J0634.9-2335?ï݀çFÊÀ+ë[³"ý*À9ŸŸ¡—[À;öюÓlú@b
#Ôñ^@Ì{n5h?¹²áØçQ?´Eæêk?ø"Ñ ¤<@ö"‹ë[-?´ãAƒXµ¿çň4íH¿ç>—"ƒ¿çÖ!ªt³¿ïÿŝƒ‰¿Î‡¾ bAGNfsrq3FGL J0634.7-2334PMN J0634-2335?ïìÓ¬ñ©;?^*CϟÎ?FãT3Ž…?CkŽPÈs?[L´r"ÃÏ?Wœƒ +r¡?ïgí$ÍÚÅ?–œ¢¸Ðª²?_«f,?r¼"Î…ð¬?'€¯â´—?"FÃòÐ3?îú=ƒmw¾?‡ÚïOWú?zõLåY‰Ò?xç¤g‰?™úüXú¥µ?´x[Tm?õ^'…?‰
 	×&¿?ŠþS/›<E?wŸè²B±?ŸÌ×¼b3?ƒ{ŸCú34FGL J0635.6-7518¿ëÅM†½ì,À;+Ë£!hÀ9"tnfæÀ<!™í|o½@ûPO£¬B@…×ÙôÓ?§zGÞÁp?ïé:g}?Ýò@úœñ@kº%€B0¿Ýﯛ
·ú¿ä†l@E‡¿égÿBÀÅ¿é»Âîýy=¿è;å¿ê¿á["{L§xAGNfsrq3FGL J0635.7-7517PKS 0637-75?ïôn«»o_?V«…t‰L¹?"ß-Ã0/?#eº óÛÕ?U*Z–E¯?TܬH<£s?ïÝw	:‡Ö?w\:류?7ãatez?,í.—]/û?pç›Õ6C|?wsR ڋ?ï¿uDQz?ƒFP'"?jwæ&)¼9?b^b»ZÜö?™™'°™?'啌e?ïýa¢ÕŽù?*gúœŸ¶Q?Ò™‹ 
>û®Ä?2˜¦@VÄO?(‰а4FGL J0636.5+7138?Çó`ר•W@8~´Øº@ÙÀ::ªù›À<[@ےbn@Eˆy`¿@¨[ü€¿?¹há?öe"?´Õ³{B¤?÷1^µ—ý@àl
ë?ïë!äVV¿ç5A•Ì…¿æwô˜Ã°Ä¿æ.ÕÀç;c¿èï9©nù³¿ï߄¬°AGNbcu2FGL J0633.8+7132GB6 J0636+7138?ïá›Yè³¹?d…3¬¬b%?E|ù$gŒ?<…†å¦‰Ê?igσ+î?b¹6hiÕÃ?ïÀÒUàx|?ŽÞŽ³,®?9tœXü3‡?OL^6´?}ÿ‹J3þf?}ºtÍ÷ôÔ?ï å•LB?)L­–d»?ojáªB0y?Z³‹®£;?—õñ!4ѯ?WWu?ïà[HB?WèF›ú5Œ?HC‡3føb?6³…Ç2W?i"Õñ%(¬?UÐëÂÑö¬4FGL J0637.4-3537?èámz½	À2	t²GÀ:ž—•}À<xŠ]¼t@tècV;¡@
Ù©T"?ÆÀéª(2#?ÃuG?Y²#?øB*aÓY¯@2Ot\sH?ïÿôÂ_5›¿Û‹4œ>ån¿ß<߆d¿ç&zü	¿ßԜåS\¿ïÿŽ‹HÿAGNbcuWISE J063746.40-353648.3?ï*½ØÚÛS?ã<Qd?j,hVÑBÃ?f^AHGð?—b·ÙÊmO?ŽÛè1/F?îæßÿOG?—°úRb~?gŒçŒÜo?o~pcûÉ? 1'=È3?–ãê!+‰?íMR,Ê*?•o]SX™ò?Š¼4õ"?{\±ñF?²=ë³ø?'؉ÇÅb?í(Iéæ!?8O?e@?Ž[
£&?x3)½í'?²òMÏ'J?bÄf(A4FGL J0638.2+6020¿Ûl›ÍYQ@5Æ՝Uæ¼À:Þ%‰ýDdÀ<'û_‡O@&cõÑb@ÿJ˜ª†Q?Ê"кm#Å?Íf¬¸ZO@ŒþùoÃ@hgÝ	¿ìÿº_⾧?ïû';&F¼¿å½xÁ‡Ê9¿æü»bJš¿ïöÃÁ5iï?Ä1ˆ8HEêAGNbcuGB6 J0638+6016?îM¤Éà±n?¢+55b‹Â?2 ºÎx?À¾Ž‰°J?£Y3AK	?žW.xTÝv?î,&‰G?¬•-ç0­?Žô"ª¥/w?š"A‡z|?¦ðl½¯À?£§±Éc¦ß?ìGúøtÅ?žú"îÒ? mÃқÃ?Š·¿ze>?µÆÙFSð?—R+çü$?í¯o›ÜÉÒ?'êÓJ¬ó? D@‰:n|?‡ûb¥3x?¤ÄŸøô\?ˆ_×»wڈ4FGL J0638.6+7320¿ïûÍÈs@9ºùe²À:ó˜éprÀ<Mš#×v@!T‡ÁªÛ@-»Å=ŒS?¹¶2‡?xmّ2ö?»£Õݗ E@•§ˆo¥ª¿ã€¹ÎÃG¿ç¡L'HD¿ë¾Àdß}©¿é£"î^íÌ¿î6±•+v¿ï«WÂ3Á£AGNfsrq3FGL J0638.6+7324S5 0633+73?ï쌌X7?^ŽÝܟúù?K܁ZkèQ?JSÚ¬Pé?Xù¶:žœ?WôÉXj\ ?ï£oYxýÓ?	(;¶ô`?JHb·Ja?`‰(œÌß?…£€¥ü?‹õKR¥‹?îÀØû¬^?'rºèԚÇ?rɊƒÌ?j~EæÄ4ˆ?¡™?ÔÀ¬?'%Ú?ïڙP®dk?`#û_—©®?Y×ê¶g†?Mq
7gäˆ?hz¹öhÙ?X´T'ž"4FGL J0638.7+2753¿Ú%§TYc@##_€™À;K§*{ԍÀ<œLŠN@!Y¹óA‰?ûø=^/`@?Ñ&ö¶|?–;֚ÖÛ?õ~…&E'?ôkڔ5¬Š¿ïÿï¤h)µ?è%¿âÙ~Œ?ï÷€Õ}uw¿åR÷Ù.Û¿ã×ýsº?Ë‹i*;AGNbcuRX J0638.6+2751?éA£ó+£?Á|ĚW˜ñ?XÇ6óÂ@Ž?Z¹µ'S?ÊÇåKÌó?Áv!<¬?ã
ys±Ñ?α@,Ï9?'_º†E«ò?¡á–ÎFC?؝ïd´AŸ?ͤLUƪ—?ê	X—•§?¢n(àS0?Ž[Ký¯E?z`.µÿ™?Åôèïª&n?¡^8¶É1?èDÈÀ${Ý?²>röêba?•ë³üˆé?'v嚽ïš?Ì/fÝP?±¯ŽõE4FGL J0638.7+5658?½Êž@4ÓDZ¢äÀ;
X;*xzÀ<›b§K3@¡)œ±|@¿¤Ùš;?ΐ¸‰ôµõ?ӜqeHO@‹"˜€"æ@¬@?¶#h?ïî¤!²Ø¿æUïÝëÙ¿é(ÒxÞ¿äœ¦°)¿ïþ–¾ßú¿ìÝE ž³AGNbcu3FGL J0638.4+5704GB6 J0638+5701?ïr.Æu\?ƒË¯$…H?wHûh5ûÇ?gGÁê?yýí4VÔ?s³éE1µ?îÞ<º+Ã?¨]Ãúò˜?‰JsÕ|é¬?•JÓsÝ#?¨¿>þ	Z?¢Å¦ÀHìÂ?í^×ÊqÍ?–cAM¨E?•^áÌ»pu?ƒ
5ïÅN~?¯cxK*ð?'Nv/5¸?íÇ,mU1?õÁ»÷?™#IêW.C?|­Y&h?¦þ8Cÿ¹?ˆnˆº¾b©4FGL J0639.6+3503¿ä^à[R"«@)í¢Pø@À:Yã|;ºÁÀ<(ѧýàk@2Pó€Ý@9{ßto>?¿0öíݓ™¿ª¢ÒÛãÐ?ëu'Ìö¾@\T‹GœL¿á˜
þEjÿå¹ÝaD"ƒ¿ì/s‹¿ÓÄ{ÚìË¿ìÈ÷?½X¿Ä	´Ÿ.ƒ÷AGNbcuB2 0635+35?îî¹5Û?°g¤t‰ü?šÔ®ÙÛ²ú?$@%T{ô?¡&¼ÿÁÎ?§ Áù˜?ï3š©]R©?Ÿ¦4WžJz?_˜õ¦)0í?s*'‡|Ì?—"yóÖ?»¾»úþ?ì[Ð
/?¡C¯Y£ù?"Z‰^)ÔV?†)Gp:l?¸
ÜÀ$ë?ž"æ¾ßž:?ï8.RºÁ?'Û׀Q">?s#Â+"Ò?gi&µá—Ü?"9¬¸3'é?1Â^Ðs4FGL J0640.0-1253¿ï•À›ˆ~ŒÀ ¤€¥¬ÍSÀ9é/bÄwÀ;õ­§m—³@""†ÖHv'?ùÜسŠÜg?»~b MÓ?¢6,"9Ø`?åÛb'Ő?ù×E÷†	¿éx¶Ë¿åªy»­Á¿àY!95«³¿Î¹©™ìУ¿ØÃd£î‡2¿¶@¼ž+y«AGNbll3FGL J0640.0-1252TXS 0637-128?âøsÖ
ö<?â­]¢Ú?jKAò"?`^ ¥)
?ÙځÏÿñ~?܃&ecî?مìSfÈp?Ë?B‹»p?ƒ'5XF1?¡××ÝÆ­?âîÁëƒ?ËVƒ¬7"Ó?æ÷"²'?ª'\§×d?"~î+1w,?}×d5Ý«‰?ÐÉ	çÃm?©Î&QP
?ܵòk&?¶Õ$*Ë*_?—5äÎU?Œ™å|P–Ý?àëÓ£úV?·SiœFK4FGL J0640.8+2432?ÒՉ±'f@!~O3Cú+À; C÷¦•+À<r2ËŸ@!^Î¥?=?÷"]wª[‰?πl÷м?ׇS±Wü@@ÅEÅ@Ìÿ¹^0¿ïþ›A9†?ïÿöµš?d-o¶•h?ȯD;CM¿Ü\O™-
¿í1}‡ AGNbcuRGB J0640+245B?ëÛ7G_Ì>?¶ÏêGH¦?s<°
IÄ(?j"0J8ì¡?¿òzÄ-Ï?¶*ñLä?ëA<à™áï?Æ4‰u œ»?dX±ËÔÍó?zÚöyèÐ?©©¶i%?ÅÙ]´èTƒ?ꏍï*Xñ?§KÅ?—YìF"?ˆ>êÒÝÛ%?ÂÖ¥1Yt?¤Çߤ÷=?íÚqÂÅk?šê'"쮆?ršbqù?i±¸¨qø?°m˜s­š?š€b§ù§
4FGL J0641.7-0320?Ø?nù:œ'À
oZÎÀ8mô¡',•À;%ºÜ	€²@Îü<Ñí@nòÇ2Y?°—Uq¡'ò?Åß_vˆš@L{‰
Z\@ƒs¢¹ÿ¿ÑyÁ¢w8Ç¿ä,0àrœ¿çG–,&Ïx¿ëymª'†¿ïy?n)ÿ¿ïû!sîfAGNFSRQ3FGL J0641.8-0319PMN J0641-0320?ïzÃ.Ľ?†ïp͝6Ê?sÔB‹¥…?q˜ÒÇ?‡""þ'?'+‡?!y˜?í"À]iÛ?¼B½eÂûŒ?GŠ8µr'?]­õû"Œƒ?¶ºê¥FE?¼6ÓÈA=™?ì±(0Q©c?¢ÊÄKÚ?£ØiR M?•Ò¸
ŠŠ?°æÒHÉd¿?šúŒ,{?ï;j¸XlØ?'_»P?cù©™à?T€îh¸I?–‡4]1×?˜ßi#4FGL J0643.2-5356?ê-ñðÀ6É/Ÿ¾wÀ:m÷hÉ™À<qދ;2@ÊkÃr†@"NÿA"?½>™~ýÈ)?'I©¹™¶—?ÓÿZS2¬û@\r˜£ÐT¿ã[m¯0Ô¿ãr2aüõ4¿ã£ð4°áµ¿äžh5s¿ë#î¼á>¿ïÿ÷1$e:AGNbcu3FGL J0643.4-5358PMN J0643-5358?ïÕΞ¤ÞØ?¢9yÕ|wd?R¹Ãá(=?€‹BáRŽð?p"B<˜JY?œ9õ€m}?ïÜC!§\?vèÒ©v9:?ZT)n¶¾?3ZÀ·L?q–õ†–˜?vJŽÁ×Ø2?ï4ÖÐã[â?€ûSyUñ?rIL_'ïÌ?pï'YÊÑ^?"ÒÒË°¢?{TˆS?ïßÔû÷ö?YÁÃ:yò?<R;¾"?+y^Ï.ь?l À '¯÷?XC8Ǽœ4FGL J0643.3+0857¿ï•y~ª@Jf:Ç|+À8Eöx—ÁRÀ;w…@˜Cz~ l@ê#ÚЛŽ?ªeŒÄ'?Æ¡°êC*L@g:6\³_@žS;¿Õd¾{PX]¿à¤¥0¦ù¿çPáïɧ¿èó­aL¡¿ëlb©Ã]¿ïÿ†}³	,AGNfsrq3FGL J0643.2+0859PMN J0643+0857?îâ0¯sR¶?—ëŠI‹V?Œe'–èê?‰wŠ¹°W ?•‡!…J4¾?™¢˜#:ß?íƒK
U'?»Op»2'?nÙämdî"?Š`óQè'?²î؉ìD~?ºÅÀ×häÛ?ë}]Þ9û¹?©›Þâ»w?®"µ6û;â?¿\Ñ#?´Ê¶r²"9?¢¨ŒcC÷d?í,Ð"1»?fÿ'î•¢??ŒžÅ?ssP…{í?´s‰)ҙp?œú"0þ©4FGL J0644.4-6712?Þê'	°À9‡ºùe²À8½CwN7À;̾&@Ü@œrêƒA@K²™ß:?¥ìAº¾
?¶ïôAðe@ì-BXj$@¾&-f?¥?Ù:!¹ä¿Ûn¤éb/¿âV<»È¿á½4ßݵ¿æTd ;ë¿í»Šàn?NAGNfsrq3FGL J0644.3-6713PKS 0644-671?ïr4D®¾*?¡‹þº@à?\9Å»Ø?gc´L"•?ëÍÛ°^\? PêrWQ?ïÚ
`£…B?v¡d¡è¾?*ž-,}õä?E?¢ª"ÖÖ?r$^DÙnÂ?uàýl1?îð+âS?ŽeÚÅêr4?"VÙ®äË?'þ–±
4F?—Ï2˜XcS?"sMàÛ?ïùXk
?;ñô…À¬?1¯7@¿>ÿŽ¯GÅ>?J±‹7Y?;3Ðt"9Ï4FGL J0644.6+6039¿à \›%N³@6ÔÇm{À:_þKÊÙ®À<'©1½n@'²'
@a× åÂ?»c òÏý?–ÇùB:{ì?à<í'hr°@Z]ÿ—¸?ïøC""~¿êxdàTi¿áZÕ¤ãc¿×ðŒma,¿àШ# 9¿ãzˆ\ZsêAGNbll3FGL J0644.6+6035NVSS J064435+603849?ïތAq!?iÀ¬!âÙé?@,?ŸŒ'5?3=Nٟ?mh®¦ûíà?hªôòèO?メj0?}'NY'¸e?8¸h¬Ú©?L
ö앳·?+r@u?{ª¦ü,Eñ?ï-æ6)ë?‡ŠY¦†ü?c¸ÄµïF?Nǵ—ò"~?ƒ*¸"'?†Ó
«SÓ?ï"&†÷D?pï5—ª2?Y~Àëï"?BNÁXµù‰?ˆ›ß䰏?p†P+
4FGL J0644.6-2853?î«£K7û‰À,&o"5ÒJÀ:Í»DLÊÀ<iŽ2]J^@ Ó ñ§£?ùdM‡rO©?ʈBZ¨m?ҁþÝÁ×@	bçcQ0@
hs[í¿ïÿ› 'V‡?ïó¯ûî|?ÀEýz¿ŽÌ¿Û'@5пÏ	IÕ·4¿æ²d ï&AGNbcu3FGL J0644.6-2853NVSS J064443-285116?îüyV
X?—Ÿêû|Á!?w†‡C`—?rή‹Qà2?š›O-|Ù?•"°À'?ï<æ¦"Z?™î¿Ù.mo?`†ªíÀˆ?uQ7~†?–RUÝü®n?˜Kܛîe?ëš96—³®?¤%Í3ì?Ÿ-S&馩?[úk"?»b၇øç? V@«ªÞ?ìɖ»>Õ¨?œ<ëàQ`è?}̌Uœb‰?qjcÎFHK?·Ö`¯Œ ?›{åÄoS4FGL J0646.7-3913¿í›_Ç»ÀáÀ1›ÜY1Ê}À:JiýʛšÀ<HÄdH~õ@–ìËÅ»¶@wdã¯ga?Ä:DŸlAr?¯'ªa4oÁ?ãzksù@	‹–ßU§¿â§´«å¿ç¼¯ŒwG¿ìc1" Õ¿è«k…L¿ïþrÎ\¿é¡–R½<6AGNfsrq3FGL J0645.9-3914PKS 0644-390?ïû{щ¿?A·ZA¡?0›·WI†?1ë=D.½?76…¼Z¿Â?6´Ç"À'¬?|"S?'•R‡9Þò?LåDøšÍ?gÿ/㒴?‰È¦Yax?·gˆE?îÝ5êËÒ?Œü|ûW1?t‰n¶à
Ù?qõîh"Pü?Ÿ6æøÍ»P?Šg"Ì1p?ï­¡nFµ?löA	N—²?a7äSžü?R~¡
û¾?€IÃõjë?i+¬gñÆ4FGL J0647.0-5138¿îi¸qåºHÀ5—Ø'sâPÀ;•YÀ<¥øZQ
@!CŽqwÛ?ú7ZYè©¢?ÏÌt7_gÅ?Âm9©Äßî?óTsۍ@­Ô€Jh.¿çX-ˆÏFû?ï‰ü¾, ¿åþ‹#¼H?Ò$Œý)¿ä6Ÿ™Û¿ÐÛPž(­AGNbcu3FGL J0647.0-51341ES 0646-515?ïÜøq$?h,þål?2™£Ýll?,‡
!¾'?pÉi—®?g¤3üÔ|O?ï²ÏqT/±?ŠSÖȆ?/¯We…Ë?C—àƒ…?:?'Íg•–}é?‰Èà¾ïñr?îw9ÊYI?‹.K_§?g-·¢œt?T´ŸŽB•ú?§‡à=D%?Š?o–i0#?ïN9¹C,¿?€/hU'?[½Ø?Tc't:œL?"‡§;ÂVé?I"4FGL J0647.7-4418¿æ^
uÀ33sâOëÑÀ:Ãf½ÌÀ<"ERðgÝ@Òÿ+ní@='¯š?È\S}€‰R?ËW\È­ÙB@·kÜÇì"@äNs«s?äšF½©™A¿ÜùÀGƒL¿ä¢­>'¿×˜Wš¿ëé¡éÛÑ¿ïÿý{ÁA~AGNbcu3FGL J0647.1-4415SUMSS J064744-441946?îcߌ¼?¢aŸ?ÅP!?'¹†'?‰^ÃÍKÛ?¦‰å…çq*?›ó¢ñ·Ç?î@$ëám?¢Ü‡$ƒi?~²IX21?†B¸kj?¨)†A¢à? …Ô߶]~?ìÁ<˜Ôàe?œ}¸" Wþ?šg¨*€Ès?ÙBÂB0¼?³\1.¸Ê³?"!$öyŽØ?ëjhHßú˜?–ÔIÇTåô? Âž×½ö?…3iø'?¼K¶i"L=?"àá7Ñz4FGL J0647.7-6058?èvÇ¢kzLÀ7ï´_½ŒÀ9ÆöÞN«À<R«ÿÍ«@ g-Å`@Wç^j?³(¤9Ù?¥ÐKÉt?ñà^åh¥@ו9?Â(mÀοæ8éU™¿ænÖâÐDQ¿ãIŠ"-Qr¿í7!ŸŒø¡¿ÑH¹­5WÑAGNbll3FGL J0647.6-6058PMN J0647-6058?ïÐÒXæf?nÓ6éç¾ß?MÈðÍ?AêåÕè"Å?só±ºn³W?l‡R
톷?ïÔý`,¡?z³…!cß?(yö©¹?BF¬üøUñ?t½€4aµ>?y§]´Ý™?ï@sA,ö?z°ßøÙw?nƒ%]zr?dž| <	?"!30‹?wL"ŸÄ¡ÿ?ï薺\¯'?Q<³	>óa?B"3‰¨—v?36
s²?bÄ8ÀæWn?NZ,iN4FGL J0647.8+4527?ã8ôœä@¡@2_–لÀ9ÏÒ␃pÀ<žßS¸@"mðÉVK@/»õäô?»ïj0 [Ö?º®?-÷?øäӛ'@¿ü¯¾¿W…ï(þb,¿åýÞó?þ¿ë4úqK¿éªBÿY¿áÑCõ"Vl¿ïÿçáüúAGNbcuB3 0644+454?ï9MR‰ûg?'ý䃩Ê?Ž¥
¿t †?Œ!ÀFtŸt?ƒž…¹?|)-˜"ê?íÖ器ñ??°g»ø'#0?'H
7´?žÜ1ïÃ?©í `"PE?§èÜÚMÎ?ëHn´üÈO?¢¿ú»9>?£Ý/©¦1þ?"ŒS}x?»ÍòƒF¤Œ?›;4&;«<?í¢Áã"?•
‡ ÚØÉ? PK·ø×Ë?Ž®9Wkt!?¥ƒ£Ž(ï÷?Š"¾ÈÜî4FGL J0648.0-3045¿Éˆ¶Ä[À,M‰ÎJ{NÀ9^íÌ ÕÀ;öJ…_Oò@/"⥧@tÁrüw?ªc;
Ȭ?À¢½¯£q@lN¡MÃ@.y¥ˆe??Û¡Ñ@ÏÓè¿àXR§lÀó¿èl3/u¿ç2,ئã¿çØì`¿ïÿî' ÇAGNfsrq3FGL J0648.1-3045PKS 0646-306?ï؁¨#Mï?gÁ¢³#æû?T>Võ:•?Ný\ƁÜ?m_,bÅî?dFsUν'?ïՇº½Q?yÿ2~î+R?7럃?Y֕Ợ?sÌñ^ßM?xÌíU€v)?零ËÝg?…öhj£)¶?yÑgÐ}?sÍ×zP\|?˜å¥2*^ô?ï·ÿW°h?ïíUˆ§è?MY ü?6>4;Ò'¬?+y¼Õ³M?_Åa¡;u?Jh6²¥Ê­4FGL J0648.1+1605¿îì˜ú.Ò@9GüÀ:îÓr&ŽÀ<cp'Iü@!Cö6D5?ûËh´€?Ë5ª†ÑÀÒ?ÃKé¸jë?÷!iÝl@š£Š3J/?æÌ0$ŠùÄ¿ïžQYŽç?ïþ"Õ½6W¿à•NEÞ0¢¿ç榒¦`¿	ã‡AGNbcu3FGL J0648.1+16061RXS J064814.1+160708?皪hm;w?¾Ÿ]¨(3?kg‰Ž*Æ°?aÆŸ>-?ГÜ	3…?¾wÏ×GÂy?à[ñýr?ɦ¾`:?ˆÍ-?ÄY?–?ÕîÆxÅ?ޅñŒ²ø?Èþªfû·³?評'‹aO?§±Ÿ»?‹ú°eJ?sá*"âí¹?˙þ¸<)a?¦•ÊKðJ€?çðš¡éߤ?°î^Žàø­?ƒG§¯êÖ¿?}–IØôÈ?Ï	ýYÔ?°Ñýº½Ø4FGL J0648.2+1745¿Õ
ÊJˆÜª@MþûôÅÀ:ð‰¹QÅÅÀ<]vâµl^@ ݁ñ\N5@¼râv?Á=èƒažÖ¿´Ã$¹ô?òÛ>µGu
@1ùeÜþž?luS¿ç
'àÂÍð¿çeþj~¤¿ÛA"YÁg¿àyVbã$'¿å®éŒöóèAGNbcu3FGL J0647.8+1751GB6 J0648+1749?æµÛäÃXD?À'âÑk-?zöä"x¿°?tjÒTÒ·?Ò(l¥ïlz?Àö]§?Ø23é^sN?Åxޝ&y%?…ª†iË?'ôw½›?ã=É7!þ?ňG]9	h?é@}XtID?¥'áv¯º?‰Œµ™à–ê?oo]ãݶ?Ée?DÑ?¤ÚæöÈcÖ?çãÉô¤õV?­äåË+ä#?'Ö6ò.õ?"'5îÿ?Î6O&gI?¯± 5U4FGL J0648.4-1743¿åNÓ¿§—«À!=‡rO¨µÀ8:êh¿;À;7SåZbL@ªšhÌr4@í"Zm3à?¥Ñl»?Ào>|<'@ãxt†@*‰
tx¿×Uˆà%¿â×nc¨¿åîŸ	›	¿æîQ Ü"¿ë1ÓíR~R¿æ"% ËÒ|AGNfsrq3FGL J0648.8-1740TXS 0646-176?íÖJ'ô¿?¢MÜþ	?x¸Ÿm?'š9F/0'?¯‡Ë5PÀ#?¡Sƒê–3Ü?ï#`Ö1º?«›Æ!œ?@àJâÁ:?`WM6¼?›ââ¸qæ?«'ø"ó-£?î6¾›(iz?š$õ'IW?"ŒÌnÏþ´?Œ9¹	Cl_?¢Í°i?'õòZdoŠ?ï¿&pÁX?ppτÌu#?7ŸÒsfÐ?0wÆÂà?ÂÊx?p 3Áz@È4FGL J0648.4-6941¿èbI!ÆFÀ9'h›Œ¹À;×5>¦À<üF€íÑ)@!M˜.‹?ü°åEi–?Óñž"S"?ÂwOWV(+?òeR…?ù(Øç7\8¿ïÑ£Ì"'â?ÊUÆ[ªq?ïՄ̂úò¿å']džg¿·ò'ÿNTL¿âù¡A-ǹAGNbcu1RXS J064850.3-694519?ïq»$ž¶?ˆ¹Ë¿Õßß??¢"¢"ùL?;YmÍ]¼<?'JháÕC?ˆ[TÆ\Þ?îô"ɵ=? êG'ݯg?`7ÎrÜkù?pÁÇõÇ?Ÿv!ØmÊö?Ÿæ"'mñO?í·§&,
?'­bÂXÒ?{CwÁ~?saÅ3»6;?°"¹ÏR‡Â?'"V"§·?ívöZÇ? 0m‡î?aùÊ
³?eVôyŠà?³ÃP~ß1u? Gƒ"Ü4FGL J0648.7+1516¿ßz0GÆh/@KÆ!·à¬À8Û
LŠNÀ;ž¡[.ú¿@!³R)˜?ú¿gJ¹?¨Ã¤¯ø*Ê?¡œbY¯ý?÷¢™Øƒº4@ ΁­¿–?íók›Æp?¯H\æ
¿ÙςŸ,*«¿Ñâ"~ea¿ÚfÝD>He¿ÚI"ÇȁAGNbll3FGL J0648.8+1516RX J0648.7+1516?í†6˜¸†?«ž'Ùëï?I¦
Ô´%?B½7ø¨Á¹?³œ
î&%˜?ªñbè®N?ëCò'¹5Ø?Àp),¤Vœ?]:ØI¾à9?r6q+a:?µÁ°‡ªã?ÀR«vö'?ì<×ðôL
?¢B(r"r??~FbK4I?p=gÉÁ­g?¼4ÚSª[?¡³5rQ?ìŽUØÕ?`héÝN?ƒ›‹OÌü?nÝó¯öÿ+?¹£í׶õ?›ôØ·ÆÐ4FGL J0649.3+2230¿åCLâB,@#<yÔØ4	À;&oþDÀ<~+qÒ
@ ×´?˜?þ·.ÕÖ`Ê?É¡Ä
†k¿?œ?÷Wó?Ì6sCš@8Jaοï{KeY -?ïþ"åÞÊ¿Ýû'¾Šêª¿á$"…|+¿ç…Õ"ܤ¿ÉýC¸¨AGNbcuGB6 J0649+2228?ëØ°¶@æ?¹Y¥ÄQf£?Tµº©?Sä÷w,x4?Àw[ÓÎñ?¹9]È͗þ?ì=O"âµà?ÁS˜S5?WkaV?g±Ú‡åƒ@?½·ÕÔ¼T˜?Á?㐃¦?êVT˜ÓFú?¤DŒ˜˜[m?‡…Lžò
€?r½‹åù™?Å.XÒÃÃp?£Zµ9"I´?íçÞxd¯h?0Pê#v?r†d˜=iÜ?ceà/ÏW?¯1Kæ­\K?T×·m!4FGL J0649.5-3139¿í¿ïY>µÀ,k-M@$³À9þˆˆ˜ÀÀ<!V˜"	]@!«ÝˆÜ²ô?÷½w$#Ë·?Á=wš@]"?Ĩԟÿå(@©)Äõg÷@	«èCZH¿ç¼ dŽõÒ¿éÛiQ;¿ß[™C]wÕ¿·ùl'ûDÚ¿×ÙÖà÷Ò	¿Õ^ŠD<
AGNbll3FGL J0649.6-3138NVSS J064933-313917?ïËç€;Óå?tþäi¼Uj?Lq¹‹05?K‡ÌBû?v~°°
¨?rÍvv©%?ï	…
…´þ?ªÎí€q›Z?H`:ðtY?`úL)Åã¾?ž\ÞiÜ}?ªÇs°]£?ío)èÅ}? Ü´ê!?lÄω?e1³–f~?³ ŠA¾û'? £‹—›?ëð
ÀÛXŽ?Ÿàœ5ñÏ?fÿŸ–?oÊ?_N'ƒ}|?¿Ç¬üs@?ŸŸÊfQ×4FGL J0650.2-1636?¸yQD1CÀî軶$À9"†AΩÀ;s•}@'/bn4;@¿~/°È?´…¢ì©Œ?¨›'Ÿgu?ò=ÂÙ.@
ï+E((=?ïèsAI¿à?Ä UàÝ¿éAΡ¹"̿塏Òpz¼¿ìÁr%·¿àÐ%FáeáAGNbcu3FGL J0650.4-1636PKS 0648-16?ìôŒ
az?²³cÄÿ?jhá…áG?b‹Þ|må?·ˆX¤¸?²¡,é>?ì?òÞtù?¼Jð
Dñ"?T‰Ú"ÿ†?kœÑÈË?½®A§£Ì@?¼꤆ò?ì¼»¼Y? ÑÊȘ¸ê?'[3i‰?†'ôȘ­è?µ—«Zo¬†?–
Ä°ö?퓼>Ã~ˆ?mëÉ¿¯?‰	ôÒ=/i?q7ø²²Os?°@ßoœeÐ?¬_˜ê'–4FGL J0650.5-2851?ïCóÑ.ÂqÀ)ÌE˼+•À:³D…klÀ<7äæŸê@¨Ïqí®@¯äë8?Ïœí¡ƒÚ?ÙX«þ +ï@$ÚZT	m@
™á*Qã"¿Î) zb¿æ}ÿ	_û¿è@›f"sÈ¿åýŒBn¦¿ïüA&PÍ¿ðAGNbcuPMN J0650-2849?ïó¯iÐe?Q׈¦C€?OrïZç¸?K]ÜrV??B>Oic-?<Øs–ú¸±?ìÕ7O³~g?¹Tm–GüÔ?Ž0Ô~»Ä¦?˜ÜÄî$^³?µ*òŒ";?·j…ynÖÛ?ì暘¦*è?1M;î¨? é¢ô×5?ßZP5?±bðÒrà?"¤¦òN?e?ì°_']·?™]q½<[?š:֜Dk?'Ód¨-Ò?³îMÎ$ˆ?—L~xQÞK4FGL J0650.7+2503¿ËÍXÁjÍ@&áõ±ÈÀ7ËUúÞXÀ;$ö%‹«@U)[™ñ?úãEš>H?›QZ™1G~?Hõ<WŸ#@m|²F@~Ÿvþ9¿"Ô#ƒ<àÜ¿È"HJ¸á¿Ûúœ~Pg÷¿Ô'")Dó¿ÞÇýM´¿ÈJì¢ÖWAGNbll3FGL J0650.7+25031ES 0647+250?ïº|†ÿˆ?z(ÂÜà?1Æ{ù?,qՋ0Fš?€êp¸?yÏmc4C	?ï¦ò–ŽB>?‹–%ûΙ?P6¹ðC'?x%œ 7Ø?"Aó…1hZ?ˆ|·õYF?íY¢ËÏ?¡ûEQ…áä?€
rn¤£?{z±Jû	\?³1;Yöö?¡ìAu4¾?ïʅ៦Ã?mó'ËÝ1?#s>M
-?fÍÇ
??z$û–:5‹?lü&½z²4FGL J0651.0+4013?ïÿÿ£¡@1Å!Ý À9ÖâӟNåÀ<Q¹¾Ó@J
ÒüfÃ@?¦›à›·?µc¢áy­?­âDc\œ?öf
{ÅÕ@ë÷/ü¿ÞÎAìßg¿à>ÌÄiQ¿à1ZJÏ1+¿àõ·§¡š¿â¡5íËJ¿çÒtvÊa¹AGNbcu3FGL J0651.3+4014RX J0651.0+4013?ï±×kÂo¦?qÕñ"¢?Sשme?I§Fw´?Aš6u–?pŠ&h"æ#?ï{ª:¦¶š?tYHRg?V‹/iÎ)?f8ßö-Ó?ŽDi"‰?Š¯!ÍòþÚ?îO÷íJ?'¥$ÅA€Ø?®NŠWôN?xPcŒƒÏ?ªlޘB?•éÙù?îÆ϶1Tâ?'Úùî"]˜?'íòz;ˆ¨?iøâVqBé?¯ü·Ÿa?€/¨ÍÏÚ4FGL J0651.4+6525?é%¡XfÑ@8ñ"<:CÀ:Zys‰d˜À<²®{¨íÊ@©µß†?þ±fYÑ,®?¿S>ìNó-?Ãb;ÉÚª@qÕ"äF@CP³¡­¿Ý
™E彿ãvõÊò×ù¿×L*ZÇvͿڝDÿŽk¿é
jKÎ4¬¿ïÈ<¿2ÛAGNbcu3FGL J0650.9+6524NVSS J065125+652458?ï"鯾;?ú ¬L'?Ž 7•1¸ ?‰™å*ü¿!?ˆ¥\{×À?€¦f?ï3˜K/?•fòšŒÑ?kÀÆFm^`?zõ¬%3@?–&ä(îT?'ÉB²Ø¨R?î(*5`?'õgOÙØ?…*q1"›?~.bfõÏÍ?¨4qéï?ð€gÖÌÉ?î^LâÅ›?‡Oüáɇƒ?"$·ò¶yl?zì"	ÑÔ? ÕÚT	‡?`~̀"4FGL J0651.5+7956¿äªjÍ(g@:®ÿ:Þ"`À;/Nbc¢gÀ<šz¿ÖD@ÌvŒyK@¶ÌD琝?À0D
û¿Äà7bÂÂÞ@¿*?nªÙ?ñÕ;0W·¿ì/AT©P¿És—ý7MÊ¿àQ½e¿ê˜YþyC¿Æ)£L¿ðAGNbcuWN B0643.2+7959?ïèºl?§'VÃ^
'?—bá½Îº?¤;W­4?uëœÇ?"^¹3*de?è0©MÓ³Æ?Ìû¬ï»
ö?À‡ws,'?ÈÞbàtŠt?½kÆ«\µ?·ˆÔ…ƒü6?꫑J4?§¶÷_ó""?²ÈAZ? ›µØLŸ}?¸‡®Ä˜?œ-UøÄþ?çÀُŒN"?¹I@œ+½n?±ÐPDâºh?°W+^6·?ÈqŸ]h?´-;±Z]4FGL J0652.1-4813?îýŠÍMüÀ3ÃäÿÉy[À;	¼AdNÀ<³""Æ@ 4'éª?þiÀ=rQV?ÎÜ垪Ð?Àÿ±%§Yv?ñð*Ÿæ»@Z²~?ï'usI£¸¿égý	«zm¿Þ?M]Uñy¿áïç"7Ý¿ßPcÛÅ¿ãΰœë]²AGNbcu3FGL J0652.0-48081RXS J065201.0-480858?ï¶è24HÃ?uÿÀ:T™Œ?B_þXÚ?8áD"&óÖ?$}sOV?uY
æƒk)?ï3ÆÅk¬?"ُ'Ôî?UHŸ ¤?aæIéšB?˜5òÑ"P~?"OöÜÄ®?î,Vç¶]?tÇÙ­§?pª
ì±-?_°T®íEó?«%P'HW?‹ä=c(ã?î3;) í?ŒzÜÃ÷M?j·¸r«s?YŒ}æ,£?« Ôb®Æo?Œ'JCZß4FGL J0652.5+1932?çÁTœm.@"	j­À:€ÈlüÀ<&D‰œÌT@jßÃ@zÓ}Àõÿ?פ˜Æ5?ߊë¡#P½@¡~4¹E1@ñ'1ó9?ïû	öùÇ?ĐK<>u¿âÛYWŠ¿ë¶¹ÐpÆ<¿ïւäY±¿ïÿ§ëkôEAGNbcuMG2 J065230+1934?Ù2æZ2ÍQ?Ä:Iý­!?¯f/Öh*?«¨VAºg?áuÖoé2Õ?ÅæþÀ?ÚotÜÁ³Ã?Ì#$´J­?Â]i?¾¯I©"?܇–Œ‰?Êêã ÿŸ?áAc9+5«?°Q¢ó;jƒ?ŋ¾®@Ų?¢Š9tÀø?Ò·Z6‰1Ñ?ªR哮ÎÉ?ãø
M$j?°Ž§Öþ©ç?ÀZ¢/¬#?¯‹gü±?ÏÅ)KH?¨îÜzˆwÓ4FGL J0653.6+1636¿íÀd^ßÍ@Û2‹m†ìÀ:(°ÿèÀ<7ÚH¶R7@–¼f@kÈ:–ÔÃ?¼= IŒ¿5óT|'Q@äO¤XŠ¿ã"¿"g¿æ(þ¦ä†¿ä_¯""e¿ã³Š§ß­¿áa{_ò®ß¿Ýé¯Ü|SAGNbcu2MASX J06533986+1636432?ë­¡jZI?³jÿۃ4¯?uV¿gÏ©?j§<2Á¹?ÀžÅë?³E=m–?ç·kžìn?ÈqX¾°;ˆ?eùëªõ#?tŠí9ö¿÷?ÐfêÎO«:?ÈZ_ãxÇÓ?éwIË/?¢á~_&-î?•m8>†Ž?{¸·«TÑ¡?Çî%Ëâs?¡|á<U±?íËl}þ}?ôýüï?t⾣?a€
£Ö??°U§°Qà,?‹1×rÚ_4FGL J0653.7+2815?ãCïX'é&@)ÚÑÐAÌSÀ:7zÀ~hÀ<U	Ĥà@G_ÏÉVv?üê"Ash?¾È"™"‰?Ðk/coæî@®þ#†î@#óï{x¿èÉà>¿j?°r@þç•ë¿Ò¾¶4žm¿Ø'=4p¿çä&Eüd¿ïþΈ°=AGNbll3FGL J0653.6+2817GB6 J0653+2816?èÄc!y9?¿ªúUæ÷
?ÃË5´ƒQ¢?º>á`'üÙ?²F|
í'ù?°¡ER…¨º?ë-Ȗۙ?¾
´hÛ@?¤d¬?a?ª†Öí/kZ?¼_¸ó¯-?·ióG)Ç?äqV†?´EÚYGî?Í]pR?²RaJ£äÞ?Á4–^SHõ? á9uW?ê³VHãï?ŸrBõÓ/?­_JiÄë?'ø/©"à?ÀQ_ÿÿ?˜±Úó—ªe4FGL J0654.0-4152?íÃ=VøŠ@À1BjDAxpÀ;%ð†æ8¯À<"ľá@ ´£¶(@å¹}d¯­?ÄóSIS0¿¦	6õh?ãC
€òç@ƒ		i
?ïcÐT@Éõ¿åÖCŒ¿è"Î1&¿Ó–[@î\¿¿á¦R_Hdô¿×V%Pœ{AGNbcuLEDA 571171?ïÊsêH«
?oÛCZ´î??—vôþß?2ɏt;'‹?x̓lZŒ÷?nøej¿-?ïu˜öùJÑ?Ž7ÔôWÄ?Bþä	ޔå?S°˜j°®?´ê‡±,?	3v8¾ì?î7ðŒ¦­?Œ%0Göáñ?pYÖr+¡O?[Ž"8«Á?ªu¼gO¹û?Šž€±xÁ?îœ!òûŸƒ?‰Ñ£€¼,?gkk;'Š¿?WxãKô?¤Ç*"?‰q)O¹4FGL J0654.3+0923¿èét$Y@—ÊÂ0'˜À:¹C•%À<:̂úñ£@ 	Ip·M4@Úÿ•võ?Ä2T"Œó?'NÓLè?ÐA
œÛ¾@"²4°·?îQ.ƼèS?¡êˆtƒ4¨¿å
!AN¿â£¹þ"ï6¿ÚG5ß
&¿æ˜ˆAØg‹AGNbcu3FGL J0654.5+0926GB6 J0654+0925?æXËÎàP?»l›«Ó«?pe—ãR,"?}QV¾f	v?ÓӆÔö¯?»u+ù=4?å<¡È£?ŧ¢
"?n×·
š®ƒ?~zLå7Ðv?Õ»Øn§9\?ÅhùÔçyš?꘥¦)…~?¢¦' ¢(é?‡U¸¥ÎÌ?rb9'¢ºY?Ä(
Üý	š?¡6Z$²?íOÌóˆÿý?'ÇZß2B?q-섴sy?aH[¡áFG?´n¹›l¸ê?'Ù½Rœ+4FGL J0654.3+5042¿å×%͈Î4@5ˆ‡"žÀ9qal+¢À<Ë­b@ê/o¯:k@™'¥R?¦æÏ=¦Ý?´%`Gú|@2Ÿà·ö@ð…×ÅÏ-¿Öü°?Mrпßv–_Ruï¿ãšÑ!Æ#e¿â³9žeË¿å«äT¨ÎÁ¿ïÿäQMÐmAGNfsrq3FGL J0654.4+5042GB6 J0654+5042?ïä©,¬"Z?_›bf_Äx?@'éÞø?6¥5!ë?g7	Xóé?]¿òF"?ï´Q!wA!?'
¿•ˆ`?D!jõkäî?VÕ!Xf&?© òØùp?*ÆPÕ}?ï±Ä·?ƒ»hæKF†?y¯ñ÷°¬C?rj-àǞB?•àÀ=ë?~~«ò+9?ïâé;ß2u?TÜ-Ò^?:"½—/.þ?(ÆÔN9ø?iÄLm礭?Sº?p³ê4FGL J0654.4+4514?"z—ÿCJ5@3cag#$ÈÀ8ë¤dζ²À;ԕ"´@?ƒ*+ù@vÞüz9'?§[ADT?´‹¿f\ÖE@{…L»@'M³çùy¿Üs k°R¿Úd_ó.á¿ä£PÂe?Ë¿ãHÑ?£.¿èåo®¿â	Y€ù»AGNFSRQ3FGL J0654.4+4514B3 0650+453?ïË'2O†?p"?B:¡äd]Ù?8Ã
⛈¨?x/êªK±?o}'Å¢?ïÅj'Öõ?}WÖº¶??T9w{?T"®aSŽx?{U¼Ó{Ž{?{o-"p,´?îô'b/²?‰ãÓœÿ?{÷`a-ï?r‹"´AW?šµ_[¡¾5?"Ìñû9&?ïõþö?d?Bc‡Íª‡?c1=Re?ƒM;Sˆ?R¨=N$J?A©x.Üv4FGL J0654.6-4952¿Ý}ãWu)DÀ3è÷‡‹zÀ:™7ÿJÎZÀ<{OnÓr@JRÃFfA@:6\³_?Àª$@ÒA?š;aµ_?×e …±…@û7Ä<…?ïàÝÆTe¿Ž×GWµý¿é´V~'ÖW¿á	Ò¾@î¿ì˜n÷. &?ÊSØÚ¢"AGNbcuSUMSS J065518-495205?íŸÝÒW?©÷T¶›`Ç?"XÞ¬®µH?{†‡FtIs?µ6Ï+{–"?¨è%æõ
"?ï"(ݖò†?–ÚQðø6µ?cE¦´S?s¨†šh3?™RC¸`øÜ?•l!ý4W?ìÄK«ÙC?›ïÑ7È°?–ïÿ'î¹?‰Üü»{?´]kzÀz7?–A<mx?îiŸòð§?†Ü6 —?ŒûõM?sªÓJ¼ì?¢0"¢B?'tÑ"²â™4FGL J0654.7+4246¿ä¬Ò@2›ðgȗÀ:VÛó±=$À<XÌ'=«@ P2O2˜.?ÿ†'+½óì?¾K'Ð|°?±ôŸÏ"§?õÓ±Þ3ý^@Y?E:G?á5av<??ã+žI+Âü¿å(M[Óem¿Úà
Fe¿ä¡C§½¿ØÉB>=þ=AGNbllB3 0651+428?ïl¡§ä½?'NšßTA?aMÐàÅ*æ?Sk»Pjk¡?TÑ®êÂÿ?htMà‡?ïjCàÎgl?•É¦Z5Í?Z³}¨mV5?j6ÞÇ
×?'L¬=0?ŽM³aÊ%ò?îàsÑÉ÷?ƒ¸p+#xK?lEã'o?U@Ôá+™? 8…/C?'bˆeû?íbÁ3jXÒ?QvFîï8?'¥
¤ß:?x.•–L¤ß?°@³»« ?½×ë¥B<4FGL J0655.4-2631?³ãç<6ÜÀ%Ý)V:Ÿ8À:u	A}À<8$â7˜@JÎãþAº@KCË0ë?ÆHÆÃHi¦?ÉÙ¨¨UI@᤽º
R@(…a8ª¿ìS^¡Ëí)?ï÷Ìàméh¿â"¤¢Œ1|¿åF–Qæ|¡¿æìãË¿ÈÈf¶˜WûAGNbcuNVSS J065523-263041?âÈ%Ó>i¯?Ĺ@2–Y-?" 'ş'ß?ÉNkðí?Ù5±Ý):%?Ĭ9ë)TÉ?îA"Wƒ?®	ja°Ó?w\ؑp¢þ?…W)¶UÎ?«K¨Y³?¬×­Gµú?éȟ½*?§³ÖJæd?žQ·|é?ˆþPÜ_µ½?Å#­jb2?¤®šq«?ìw:›yë?'PØçM(?–T몶ƒA?~›GÅúTà?¶°ô°vÔ?'Aã?¢4FGL J0656.3-0322¿î´¶ ôþU¿Ý
ÍÞo·sÀ8S&ùz«À;‰ó3hã@ð¶ÛS@WwJº8v?­\ãã?ΔBWC@´'¾‹Áj@°'¹%{¿Å)̗Àñ¿á
Hï]¿çåàϹW¿é¤''¿ëÆ?wå¿ïÿù_|è3AGNfsrq3FGL J0656.2-0323TXS 0653-033?ëÏÿ¨®à?»'E¯ø?ºû¸´lÔc?¹º–JAÝ?š(Šrr?"ÝÑì"?ØùÝdÅ?Д%4¤¸?¹€Wם?烃N?àSo/Êâ‡?ÑØÅioV?åŽçdÞ¡9?±Èl¶"_U?ȸdÇ­?¯5ut÷¥3?Áý¤Øu~?¥ög<@…?Ý€‰Có?±¾~ˆ^Øô?À´)ôÊ®?¤m˺'÷¥?Úõ%Õ|V¹?²+ÝO¯Ê4FGL J0656.3+4235¿Ø_‹¼óL@2Ó~=ÁÀ:³pޏmÀ<P%üu@ Ë­R3(¡?ÿyó$÷0?Æ>oçÄtå?º¬³æ?÷5'm,S@œèwx1•?ïù-Œ*E¿åùy¾‡å'¿Ñâ<xm¿áÄcq¿`¿æ"À%?nçcsdH AGNbll3FGL J0656.4+42324C +42.22?ì׬€é~<?§Þ/E?¨?e+Õ¨3Ç?W_æÂ\?¸™C2̅?§ª°J¤Ë?íµ3©}?ªÖ,ÝAÚ?Û°±"îø?†Iå4Jè?°ZW¡é?©'üî›"˜?í;=$6?˜{ãÇ)ͯ?{c€¨˜?jâi'v?´oÞÞMlÃ?—&kÖr¯?èe®·­ƒ?§ÞûòeÒL?•'íó±?!?èIJ\ÉL?Ë·bÓÌ?¨šøž2Z4FGL J0656.3-2404¿ëËÇû#DÀ#d¶0©À;("VÀ<dYV³jü@ €õQ%aŽ@ŸKÚÉå'?ÆrÜV¿H¿ƒ¢õ
ÐY?Àh[3,}@aþÍ¥æ¿æCé>GŽ_¿äڔk\om¿èI.p•¿£ÛÔQ¦eÛ¿ëlé7fž›?ÁÂkŠg¢|AGNbllPMN J0656-2403?äÛù¶]?ÆfÔò"?s:'9¨«?jo7^9?×£_oùòú?Ãg¸ÊÄ£?ã4m±Õñ?ÊO0dÉx…?]#)ö»?mH'"?Ùz²]b?ÊHÎĉÎÏ?êˆ[zóKŠ?¤NÄqLÔJ?ŽÈÿ7Ÿ1?|ÿ+¡SN'?Ãò?Wã?¢ú±}6E?ì.Ôº Âà?¢Ð÷i™?w¡Piáf?p,oSª?½E!#Jñ?¢ŠïÝ¿ÇC4FGL J0658.1-5840?ÊÂñRyZÆÀ6 ÝDÀ:Ó"d®ÖÀ<šU¦$ÂW@Rmⱑ@S»¹/?Ã,hÿ?´ÂÖÿ«œQ?ðΩ+Ç?üäò7ëSÌ?捻å'6¦¿Ñݦ䱿ÛY—á]¨}¿ç¼o¢OJÁ¿æ¢nŠ!V'¿Äpêù³Š±AGNbcu3FGL J0658.3-5832PMN J0658-5840?î™ùMÇ<Û?˜¯ÀIí§?eeå‰Ã'<?Z=‡ImÍ?¥
Êïù)?˜ŠžÊk?îhÿ5—M? >#uÐÝó?qLÄN÷?r[תõ?§MÆ4¬G?ž«ÖÛÜ9€?í`õ´Ó€?•€Gz2l?‰ëª;­3?|~¤û¤nS?±ºáÂ㽕?'GÌ6[®¹?ëðÄ%wÏ ?–¦Õ¸?œæ§•qÀy?…ð¯›X–?¹@4îåì?– kx:›ò4FGL J0658.2+2709?ë_ߣí@*ÍA·ZtÁÀ;½x›óÀ<…®
iæ@M†›@ì†;?ȌÇÀ'?yuD½®¨ž?ªLõbSmw@ÄØÆU9m?ïe€Âø¹¿×Ñ}
§¿æ̝Òä>¿ÔÊ#$G]¿é"Ì«>Þ¿Ü#"$ÓAGNbcuB2 0655+27A?î({Œ?¦ÍÀ\òÿ™?d5Ñé…{?ayW^Ï?¬4þ™Ø§s?¦`ºp¸ë•?ï#îhïÆæ?£¢%tGCð?E䕰ø©ô?]Û\ŸÍ?šÓ4]ý?£_Ƭxƒ{?ívÓKÿÊÕ?–æ"?ÏÝ´?A)9­ïÈ?rw|×Qºç?²!@xËëc?"ÅçrâY?ïYrbV-Í?v:O]½n¥?e3½Ü?P«sÔÕ¶a?'/M=šB§?tßÙ`9"¹4FGL J0658.6+0636?ëó'õCA&@j¶ÂŸLaÀ:R"ÅõB7À<+°¶ì'@ °jûw?ÿKXÃæt?Ã"ÝûsS_?¡¬ØwHP?ßmõܐ/@Ûäkyö'?ä'6ÎÉ&O¿ëów'1L¿Òˆ:̄¨¿Ú#ìnRÄ¿à¬![š[¿âžf½¤:ÝAGNbcu3FGL J0658.6+0636NVSS J065844+063711?èa<…P—?»*ùi•Î!?yd	ÿT³?pžÁn'?Í®"˂Âþ?ºì™{ï•(?ãÿ_¢n>Ü?ÅŅ?p{C-~i;?€Cû3­?׿S®mˆ¤?ÄÆÿ)}9å?èg"HsÆi?¥¦}8.8?'SBP?wYx¢	º—?Ì@äuæãi?¤_©vM)?ë¸:]âèF?–ŽX¿³
É?'`´-ÂÙ?mޞ_¾å?¿ò‹0b¤?–]xIÕQï4FGL J0659.6-2742?ïÿ¿[}²¼À%/UÞXæKÀ:3Æ&À^*À<3"'ʘ@X‹®õKq@ÚíÜçÍ?Â\ÉŃ"?Ӑ{xFb»@íÅÖ8†Y@‡¹Wzf?ïû7mª¿Ü´>¥¿ç(Ãm¨z¿èjÃQ#¿éÿcøÍܗ¿ðAGNfsrqTXS 0657-276?íú:¸…T¶?©ÝR'9?ê2W6Êq?,œ'1]I?§ç;LOu?¦y·ŽTÈ?åµü£{,?Ê"( ÷÷?–f ÁIÎé?¡Òï8ÜÜ?Ó-¤Ø¤lº?ÉX
61¹÷?ç>lÿÿg?­à?Ÿ~v¬?¹Õ;šÆi™?¡ñߣw›?Æ®6`͚?¦Ñ«\§œ|?ëTºiž+?šO]-%]ç?¤2¬"¼™?‡~æòòS?»\ÌIœ?–SzòÞ4FGL J0659.6-6742¿Õú
å#ŽÀ80…†"À;Z©Jç"ßÀ<¿<ÓÅåR@"0ü@ظ=?úƨZý|˜?Æuøˆ‡?œãg‡½gï?×p§\û®@á*ŽÉÝ¿ÌÁ¬­O"¿ïúeA"_%?ïú¹¤ÑÜ¿âït'ƒ¿Ü»©ú9íb¿›…
›tAGNbcu1RXS J065933.5-674356?ï…Bé…?ƒ`F¶½Æ²?9Hüi¨?/±À¸eêH?îç›bQ?ƒ)';G	'?ïG ¦ÜR?–4kA¹¥õ?Q9Gäxºy?e~bç?–V¦.3«?"¿^õ¢[?íî·'6 ?'±xS¾Ç?o>}çê£?`šX?¯ ¦ø]ôe?µ?Gýë?íæÑ¢Š?¢¬À">n?Z©ipñbé?YHh<­"1?·n)»¯&)?¢
!ìæA@4FGL J0659.9+1709¿ëS;Þe@#¥ß"9çÀ:4\|ؙÀ<‰£–@(ÄBd©x@#«äøê?Áï,ž¯N?¢_ä°Þ?ÝÛB›Ûé@
=‰T'¨¿áë5@L ¿æDI,«¿æêò®~¿çbår¶¿ë	3ðÈT˜¿ïÿHë+\¥AGNfsrq3FGL J0700.0+1709TXS 0657+172?ïÃiƒÆ?"Á"\$º¥?`šCR¥gå?QT´ÓÈn»?šì_(zÚZ?"H-Öóð?ïLBÒì¡?«ì$
ë=?@.ü…f?U)èܟK²?±Ž4ʇ"?«Í+«ƒ?íÙmvÝÈ?•ÊÇ6¼Íù?ç*Ð?pÜvљÇ?®lC\1iw?"œëwN?ïe¥uÜë?vc1›e<?Yæû	/¸ç?CûU¼ÔS?'¬á"Ï ¨?us}¤/"4FGL J0700.1-6311¿îÀ½Þ%oÀ7·ª%ÙÀ:±ñNŒU
À<˜M×ú'y@ )ƒ:1ª?ý'-ê
Ë?Ƃ_UÐìí?ã©'#V?ýÖ—Péý@ô
8"x¿ì(ǀ?ïúªùš‹¿Û["ÀĀοÚkaýËó¿äãacÈ&¿ìó)WèbAGNbcu3FGL J0700.3-6310SUMSS J065958-631238?ïÏ"ßv[h?pgðQޜ?K¥÷o܂?CNRƒŒ(?u
»…äP–?n£!=m"?ï"ÝT©ÀÛ?ŠjÝÔ<"º?BØ¥fœ]›?R¸Ô
0ÿ¦?‰› &b?‰:O\–a?ºlÐ?‰ïÿ‹¬ é?oÜÖj}ø?`ñqðiˆ ?¤è ±Sq?‡Ýe$
}?îžæ'ß?…Â10tù?y>÷¯È´?e-…Æ–ý³?¢ö²¡åñ'?"FHL¤9t4FGL J0700.2+1304?Ùhš%äÕ@h>]2àþÀ9æGÁ_±À<(É Èb@Þcðë: ?þ«rßñm?ÀéðÊ1?¹ù]ú\'?û±ƒ›*"?ñºØ®'_?ëKg<O;§¿åj(3¦¿àà Ç`¿ÕZ¤k¿äÐeÁ•a¿Öi}±ÇAGNbll3FGL J0700.2+1304GB6 J0700+1304?è°r®@0?¼¢œ¸³°? ý++¶?uË÷ÀÏãÌ?γ=õtL…?¼p¢ˆþ?Ì6Tz¶/?Ã'Õ±ÊW?¸üJÌu6£?À
Ýy}=ã?åÒá‡Ãµß?Å,W5®–?èÉÎ?¦
ò1°µ?"àïsù6?|ÿÞ
¬"]?Ê?¢Ù+l^?¤Ý
·R	?á	FÔFà?§¬Ì^©Ôº?Á¥.šNJ?¡|ŸÊ {?Õ-ŸÀŽK?¥ø‰ÝKlW4FGL J0700.5-6610?îzƽMÀ7–6—lÀ7àóÌëÖ}À;n,Ñð"@zrè)õr?ÿlV…GÒý?˜´C÷ä?³èù~0²z@H	N][%@J	99²~?¢‹>šÖ—¿Ø}å,õ,¿àŠò×ùP¹¿áQ¦ é4¿åó`	€¿å™
Æ(ÄAGNbll3FGL J0700.6-6610PKS 0700-661?ïÜ•P7?cÁœ#ß4?2üŒËÀ¾?+‹ö£Vå'?pҕÁ(?bñïùÝQ?ïˆCÀDØ?ŒV¶Wžq?PŒÔ3rÉF?g™¥Õ*0Å?‹ë"‰€pë?‹9KG>å»?îÝÙªFüº?'3)Ò·ÅÉ?"àDþ×?ƒT<­ÇQà?™Ô¿" ý2?‹h¼kâ§&?ï'4HßcÙ?t)¸Ï
?\µö«½P¨?M[¡²¹?‡Ü.ò¯_g?sL5Q¥¿4FGL J0701.5+2511¿ì¨Jžoþ@*ˆšgó
À:ñ/¨;ôÀ<‹5RÈ$@!""«þÎ?ýïüÍE˜'?Â`#×·¿"€-Hâ$?ӋªãÃß=?ÿ8·§ ÀÀ?ç–_½Õ¹¿ë%d`ãð¿šÚ}xg¿éCN¾ÿږ?µÝ´¦M¿Û'@dtßAGNbcu1RXS J070132.1+250950?ía.¯7…?°Ei¢øV?`"×Ëæ?V•ÁzX$¨?´usÍè´¬?°*Ú/Ÿ	?èVÂ7@ž?Éà?¯g?}qÀWT¥?Ž/è´¿‹³?͹i D¥?ɘbtŸ?ìk|Тà?¡ì°¤¥?v"D&u?q5¿ËŸv·?ºuFú¢Œ)?¡2÷¬Ň?뜈jÚ?¦#ŠplF!?kTz]ËÏ_?f¿¸Bð S?Á ÔÝhS?¦-ìte4FGL J0701.5-4634?æGsJê#À1´ÖÂïÔ9À8ýë7ñÞÕÀ;íhò1á$@àht³†@‰bI¡3Â?©¾X»æ?Äâçxb<@4aQJ@½©›ð6¿Ì~UE¿]¿áŒ†'ø¿å‡)õœÏ¯¿ç7?#Vq¿ìíÝ|艿ãšÑ½woMAGNfsrq3FGL J0701.4-4634PKS 0700-465?ïîû*µ™?˜g Ù"ŠS?S–_åÜ?W÷IÖö?Œ7ížò³ö?†`Ñv²ì?ïÄaæ•º?'œŸ­>Þà?>_T'NéÍ?Wx»;ð ø?{é;Ð3ö?›ka6˜?î@Ž¨Žú?ZþûHO?'ZÊÕ-
?ŠE{Yǝ?¢É'ªõyÅ?–ÚJ®ÿJ?ïÐ\¤f.&?cQÑc¶B?R[''š?ClªÈTj?s:ÍG"GY?a€qklªÁ4FGL J0702.7-1951?ë4¯ÜÉfˆÀ_9K{)À8°µ "µÀ;q׉¿1@êwY¨½Ï@ ºK?©ôr-Dé?¶Í´~La-@
ۇz³%@b
Ë5¿ÐìK¢ë§Ù¿àÏ9#7<­¿ÞÕPߖ~¿àèuÕo2¾¿å,‡m¹—¿æ¢Òþ?5 AGNbll3FGL J0702.7-1952TXS 0700-197?ïƒä†*{?€œá3º›¯?8Ù·Kݞº?3Ü#¶†á?Ž@»3!?€gîÐӅ	?îWü²>èZ?®±Ø1$2?9Áó'hé`?R38Ü«ó?ªL°õ¨Š?®–3+t¬?íÙø‹cžŠ?— "ÉÉ:?ñ.±?t+P—o?­ùMzk	?"ѵ¾i?ï'f"Z°·?tÈHµ_ù‡?H1ǀý•[?7ª"#¦!_?ã>±Cù?tdBV^˜p4FGL J0703.2+6809¿î×®pHðè@:.Y¯ž¿À;Äp/=mÀ=y@]¾!@!m›
à?þÁX$"D?Í¿9?«BNâ™ÆC?ß:#<p@#_•'Í¿é(Qû,Ý¿ìÎÛÐuι¿¦èsFs­¿Ý»ˆÂ0ç~¿èóá
Ìq?Øߓ£áF,AGNbcuGB6 J0703+6808?ïMmp@Þ?"wû0j¬?Bö&æ€ê?BšáXFÓ?•º ÀÊÜê?"%F¦0¢ë?î÷@p‡õ?ž"2«	9?aˆ3Õ&c?pGXçðÆÛ?žæëŒÆ¹¢?œ[´óç
?íÌ"´Äk"?"TÁ
÷)?r{÷U;D¿?jÿ'¾aD'?°w*äˆï$?'üí)A?îÅ.ºâ[â?ç'èfÿ?U¦4ßçª?LŸR29?¢ÿⱫBž?ïʝ">\4FGL J0703.2-3914?»L*%'—À-J×ùP¹VÀ9Àø£lŸÀ<6¦CÌ«@b'vŠv@|_ag?´ÂüÿÅr?°uŽbÿd?ûBJÈ{.u@Q&úë™?ïñöó4¿ãå"~°	H¿â´½ý&¿×ÇÚñR¾¿ç$¢¬gÒw¿ß	žs`AGNbll3FGL J0703.4-39141RXS J070312.7-391417?îÑL]vâd?'&Ó7B?q,s@Ïa?gý‰LњO? Å«Æ)¿ï?›A"â?îñ	Ôc¦3?›:Ïz"`<?l"CgŒÃØ?v‹i9'Å?žN=™¡?˜QTÈc"?ìÙFŒ¥¢¹?›®ÐŽ/m?‰î»ñaž?xeMýð+??µøƒT½ù?˜…PaÌ´á?ìtï¢P#?"æð4Ñé†? Tª|›¤??©Õu·y?´.~˜@™þ?GOí<óz4FGL J0703.3-1042¿ç=¡>\9ÅÀ'D`'!À9j‰r¡À;HlÞO¬@¶6]_,@5£]gº#?»€;"n?"‰y­ò?ÙSËäÅfý?õ˲BÝË"?ïìfZ§ìC¿»ª¾–9y¿ë0Ď9ê¿é;(àsó˜¿Þo+|/¦a¿Ô‡B^Ê:ÌAGNbcu3FGL J0704.1-1043NVSS J070322-104426?Í.'ošr?½$Ãò±"?tܑÛ:ŠN?pï3òh@?芾÷í¤N?½kß/Þú?Қ®›ß_e?Å&èòŽ?ˆ·@‡ôã?'…=¢€'?æO˯ð|Á?Äïâ=}5_?×RqBcÃ?±T»–9Ý?®xp&Bã ?&7vK"¯?âo@\jGì?±	½Êô?ٚyv²ö?³6XKñAk?®â*B¿$?š&s+V†à?áD  }¨Å?´ ^ic€r4FGL J0703.3-0050?Ä8'©Ì~@ø/0oÀ9ˆ²1@ìÀ;—'?2D÷@dn9ïdý@ƒ¯à,ûâ?¹nÓâ¯|?É'ÄÀ
÷@~…vÌå÷@
Àöäxe¿ÝO©@U°Œ¿ÝÖ
RÎÙí¿áú4CÔk'¿ä>¥¢fqÏ¿è1áÏh^¿ï÷:Êi²AGNbcuTXS 0700-007?í
ßÍ÷‰?«ÒÞ¦}7?òîy½òH?‰—øÂQ¢?³lEñ×ÿ6?¨TÜOœ#?çø˜%*‹+?Ƨ_ÏÎñ?~.펴óŸ?Œš[‹¾Ø?Ï,'þà+¸?Æd¨•Æda?ëDîàw~?¥[cOë
 ?£í?ág¢?–:NÍmòž?¼	'_«=?Ÿ¨­oî©?è×ã­½,?¢ùëä›ßå?•à«®:Ôs?|‡'rl?Éä[°Á?¢TAE‹¬4FGL J0704.7+4508¿å
+Ž¼=@5I˜ˆøÀ:ÇG'u¦À<hÇñ›¹/@ŠÒ¬_Å@@Ÿ}i[?ƲŸzQC?¸fœ«fK?îÑ;ÇVkG?ú"#xÕÿ¦?ÑØ	âx¿ã¼Å¸ÜU¿åX•Wëy`¿ê	âÂW}ë¿Ö"%>(¿ïð4í0EAGNbcuB3 0701+451?ë&gïP°X?¾•Œ¸­?ymŠ­îƒ?y¬ÇÊå\?šóòÏ.?¾Š¦¼Ê?íÓY6Eè?±"U"Tñû?<ÐW¡›û? ¨e·Íh?³1 ei½?©{o?íÉ<ÐE?˜oÒ[¨[ó?÷m69ü?ƒkµê°g£?³{ÚÒ;<T?"9¶}âA?ë$è(g?œ
 =ö+?••Q±5Áw?"žOrB:5?ÀøÂ)8Î5?šÿÃÙçâÛ4FGL J0704.8+4907¿ÏtˆŽÀˆØ@6BÅ;ËÀ9äz[ñÀ<8>gCÛø@¦¼õ¿4^@'8å#Û§?µ}€´Elq?Ö=C­Sá@
bô ά¡@.-ú'ѿ͍òÇ]L6¿âu۞÷§l¿ärB¬^¿éÍÃ\Ⴟ彵½¼Ž'¿å°eùRAGNbcu87GB 070112.8+491056?ï9M¶-<™?'­Ýi7k=?u1—òïI?u¾÷¨f'¿?"‰å[°ß?NØUh??¸áµ?"·óåܱ†?MŸå«òn?^j;ÖOx?‡@ßù7üg?'ü`xóXà?îՃú¤8?Š\¾3S(?pT˜5Cè?záx(aïO?œ—t4×*?"D@÷¤Ú?ï'Y‰ùSr?qeƒÀÀô?c§éë@"ì?P¬tÉFù?Š£Û9?pEwí¿Œ4FGL J0705.7-4848¿´õ1ÕAÀ1Øc8´|tÀ9Ö­ò2qÀ;úˆFŠþÌ@âs'?	*@Oï0l¯?¶®|Փ›?Å?Û¢¨‹û@
3Xòà\Í@½^Ä»?â—m¿öûu¿ÔB±Á¯¿ãx†YJôñ¿åûŸíp±¿çŽëUN.¿ïþu]AGNbcu3FGL J0706.1-4849PMN J0705-4847?çπk"?½:X'R?À¹Z½Ù£°?´±)ŽIƒ?À¥دÊ?²¬M1™Ä?éÛ¨-Ïíâ?ÀÕõB?µùšÜ©3 ?¸Ç—y·±?»)#´×]R?²p+\¼‡â?é¶
*Ò?®‡*v–?¯ùÚcÓ?š ·3º«??ÃÒááQ»Ã?§×,A´.?ä<æ†1? J9"œFŸ?½œLå]?šž°;"_¬?ÐB= ͺH?6
zå˜4FGL J0705.9+5309?î¡k➒Ÿ@7€ZpŽÞUÀ:Ø	ٝ•¨À<³Ð¡m£r@ÁÂr«Ä@'6~AN?ÁÂ˗´'?¥ùiãÉh"?åe'
@ž3ƒ:1ª?çÛ-¸Ÿï¿×å°¿åï
¿[J)¿àñ¦&oÖ¿áúw?|—«¿å¡àåÞlAGNbcuGB6 J0706+5309?ï¹÷(ÆÀ?v&i(æ§Ï?TêÎôËÆ»?G½ñ$Òà«?}Éîi®s?u0I~öKÂ?ï¦uKÀRç?…ý6z?B3hS Ü?PXpº
&Î?…?vŠ¹´<?€….C^ر?î–ÏGÊÃ@?‡4(¨sEÛ?t¼¹¦Ð	?_û¶õP?£û‡Œñí?…C'JGå?ïoà‡?qWà5?pRáYi?U¸ø¥ÌÄH?‹Þùȱ¹j?ny)ª,–Ó4FGL J0706.1+0246?´%Q|­!L@.beOæÀ:ýž5	ÍÀ<SôH;Øô@#½ÙI\ë=?ù"¡ò?ÄÚUv
Q?†o*bÝ£g?Â`|-Q?ùœÅˆŠÓƒ?ïMú^ÖO-¿ð?ïÿþó…õ?Ôr‡qxé ¿çää†&ö?ˁ%D@çAGNbcuNVSS J070610+024449?çv
ô}¹Å?ÄܘçN-?Pfcž¥¸ë?Dê•âÏýN?у³eæ½?ÄÖáÄ	ñ?ßï³\¥­Ž?̚I&ª'P?Œ#)^·?¨'~–K7?ß/3Xiœ¸?ÌȘ*ˆ?çûHä"'€?§|ñ÷¢›$?‡þfâ¢L?rHÊ®9†5?ΒöKÕ½?¦è`¸Í‰?äÍà¢~Òú?º $¨õo?–Qåç`*G?•'Š6mÎÞ?Ôÿ \ŒWg?¹æ Ê\]@4FGL J0706.5+3744¿í#`Ê<œ
@2üð¸,,À9'dö#Þ,À;Ӝô—ìñ@ÍëZ×g?ü=³¥Ýu?«–3Þ~Ðë?°rõjû¡w@ƒZ'ó@=«2ž7ä?ïæ
öÔT¿Ùº"ÛÍпٔPdF{¿Ú&Y›|Ȩ¿Üž^$x…M¿ÞË(~»ÈAGNbll3FGL J0706.5+3744GB6 J0706+3744?턖žÊʕ?§áÌ2G?ƒ-*ªOý°?y▸"úñ?±u¥´_«›?¦oð§Ð—¹?ì@Âûm"?¼ÞnÔ#ƒç? G«Má4Í?«ÞÈ?{%?µÖ}¦U‡?´ƒ©ìFÁ?é×Íá¥dt?ª">DŒú? %.ïÅç?Ž:žà^;ë?ėh­®|·?§PÄóÅwû?çBÛzتÿ?°€5Œ52?¥ÛékóGù?©?+Àûd?Í}—¹ '?±P{³ä­%4FGL J0706.8+7742?»žŸ¹yC@;Gy¢ƒMÀ9kQÄòÀ<,=ÐE'Q@¯"}ûÙU?ýıû.·?­òŸïV?¾kdÒèoÁ@"ïï@Ÿ|󛘢¿ÀµÏš²sZ¿Õ‰æ]Â}é¿ÜÙhrLN¿ÜlÅP+¼¿äô,ø†Žû¿è"3ÿ
zAGNbll3FGL J0707.0+7741NVSS J070651+774137?ïàUGU¨?c'Qoø?QikAZ-?IîNžšþð?fö+ýCt?`d%¡N?ïª>—Ýœ?'²ÚýFȶ?FÅÆ<ï'ú?Z‰ÞÂ?"ý¤Ê)?Z–­;~?îÎößJ¦\?"
‰a
h?Õ!J'?‹ª	P'ø"?–6"•&?†•ªqogw?ïÓ7‹ih?\‰ìoэ¹?E1e¥"ø?3"Œwçï?s¾
½ê&?Z"Ù³'4FGL J0706.9+6109¿ØâµÜ	E@9^=áâßÀ:>pɖ·gÀ<'UÓø@¬¿y4t@,ÅZèƒâ?µ¢7¢Ù‰I?ËPÿT'?Ö<á>iÈ@"IX¹"?ï &Ö@¿äȒ@	‹¿ç>-—è¿r¿áÒ6™A¿ç}§á¿åmü\ÝQAGNbll3FGL J0707.2+6101TXS 0702+612?ïBwôzó·?Ž´"ü×´?dFSpÍ59?U·êÂîv?•(7‡âj?í£ìYg?ï8QUz?ˆ`B4P '?P:*ù';?b 	Ȓ+ì?‰ø¬Œ‡®à?…½ÿ®ÿN0?îܲ¾±ã?‰t.&?pÃ5ä¯(?`d
´Œþé? wW?†ùÖlð?ïdº'ª‰!?rÍÊƔlÎ?}ôîyA­Ž?c(Re1ͯ?‡Öä¼á?kC²¤W4FGL J0708.9+4839?ÛçUnòQ@6Ɉ;£D=À;IÐ&ô`À<Á½"¨™@!¾¢ªdm?ù~{?ÑΝœ…?Ãfmé~3?õslg@8Ë0šÂ¿ÛšÚŒ¿ïÏäM?êÏlº=~¿ÙèêÅ[>j¿ÒÝWžøS8¿ÞP?þªJAGNrdgNGC 2329?îvB!i? ˜LW)Ð}?d²­;ËÚB?]q­ÃþE?§P´1KÓ? ½,%?ï¦t'î?›þŒåÁÅ0?\PíL[??m4+JÔ¤ô?œf.|¯v?š³]ÄdÃ+?íŸk`oJ?– )Ãa?qüz/Z?\àügÈ_?±÷dÝ\b¿?•WÑZ!(R?íäŽü$È?•O»‡÷?Xô—kþ ?V{~AìËi?°wµÂ`Õ?•ýˆ­`4FGL J0709.0+4304¿±Äž¤3Ð@5-j½ãû½À;—ߨq£±À<žÌN!Ì@ N33²à@tÛ>—?̳Ä=19¿…˜ô`Ãô?·B›îœo@´h"ÿ‰¿Ø>\œŽ­¿î{ ŠN£¿°©»¿xS¿èä§՟Ú?¦RCí²1¿ïÿ¡ ÏAGNbcuGB6 J0708+4306?îyé¶Bä?¬"@!†?b'ÀæÝ?j2Ø_Û%?§>èžcá?«ñÓWeýK?îÅHßÌÐ?©F†Íl*?a<Íå#ë^?qo7Æì˜?¢—¥0`ôD?¨†eð9D?í3ÚÌ#?›TòÿëÐ?ãäf«5X?uœ€ú÷Î?µH"ã44!?šFwL<Ÿ?î°ºÀ˕ø?*80eI?;[@v/´Ú?8/ÌUŸ^Ý?¤½rZA?(¿Æà,74FGL J0709.1+2241?ëÒê'äv@+ªºà;>šÀ9Hôá¾ÌYÀ<*2	@Êi©;ù?ÿí…tH§9?¯ΠÑ5+?±k
?-½S@t–'äZ@D!ÂóZ¿äÒ-^ÝÛé¿Üeށ*7¿Ýk¶Eê¿áK—þŽæ¸¿å_(뱔¿ÙQQAGNbll3FGL J0708.9+2239GB6 J0708+2241?ïíŸåV%?[…¹•å?&RÂs¼=?"Ò) ^ŒÌ?`ûÎóyo©?Zqp=ìãˆ?ï¸>Á¸	®?‹eÖ]{©†?>\­­¸e?Q£r?… ?€ýj)à&s?ŠùS" ?.?ï	hohÖ?†
‰\‹?r)‰\>ú?p<µ—ÿu«?šH»Õ½?'ËgÃÆ
?ïÒvìêO'?`ûÈÅbì?F)lt¹Ï?5]dØn·È?sÿ[üAJ3?_8ì¶4FGL J0709.2-1527¿é˜§7«¬°À	0$öYŽÀ:–æ`ò‰À;øªLb@!€¼&'?ûÖNUÎh®?Á˜kܜùu?½j§=Ç
ì?þì¡c'v@Y1(¥¿ïÿÝ/ñ_S?ïÿþBe«+¿ÃGahz½¶¿ÇeöÔÞ¿åK
P»Ú¿¬:XŸ¯AGNbcuPKS 0706-15?ï
 ªÛª ?"u·pù?NÞxVf+?HemÉHˆS?döá׊½?"5
yí?æ>mèéa?É"Ùzx?[A;è¡MM?]¸C¤?Ógâô
‹ñ?ɍÿьº?êùäu'ÛF?¨-×ÿå¦?†ËI§;?uÈV
ي?·!u!6?§?žÒ~?ë,£ÑV<?{NY.J?†u)Å5!?rù]2T¤?À›úßS¸?A{^
84FGL J0709.3+0540¿ê'…4@@W_bf'À:7a=1¹¶À<1REG1î@KÓòZûÏ?ÿ»°åæyF?Ä@jS…ä?¸HQÓ\?õ:ðFN˜ê@'P(as
¿ïþ`ù?Ÿ?ïîLC¥q>¿çØ#­"2)¿Ð®#¿LÜ¿ãˆ$A'è|¿à8L­W¼AGNbcuNVSS J070916+053901?\;`?£³ d;?SIÙ¬º`?I¿¦]#vŠ?­üÖ<Öy:?£Ì€ã!?íp-¹g?¸	:dr?Mµ"}A	h?`j!+	¬o?´Cëk:E/?·ð¾?"†?ëwÈJ›?¤'z>çøC?†
ìl‹?tB$"G?ÀÀ~°Î?£:ìáÿþ?îÔVjêt?'i½˜¡)?s:æ²bO?] ÷{­å&? Zs<{‹?[tT°E³4FGL J0709.7-0255¿ä¿ÞíCÉ@åc>"¹†À8†à66òÀ;q¡3ÁÎl@of×¥mã@¾::ŽqG?¥­ {\?±¹_°ƒ…@	•õB6Ü5@T84ÏÀr¿µVz\'}¿ß| $"I+¿åŽ¨orŒ¿âh‰¡~ëC¿çä¢ Ñ±¹¿ãHhÌAGNfsrq3FGL J0709.7-0256PMN J0709-0255?î4×ñîÒP?Ÿ"<e?Pjd¼aà¦?G&f(¢Ï?¬/-»/Ëô?ŸqW7‡?î«wbY?«û×Z:d?O¢—Ï8±!?jBU&L†?¤ÉÿvñGÁ?«·#Èíð?íÁ¬XÆÞî?˜ïæ˜IQh?"YñtQ§n?w8×å}³3?®Î¾}§Y?–
"ͯº
?ªŠ6?rö^³ù^?Lڊ]yZ,?8ÉíQüMÏ?‡ÄìԅÝ?rm;çÚ}4FGL J0710.4+5908?îI±Û‰.@9lÀz®òÇÀ9ºÑ4:š0À<6ÙCӔg@!‰Á	u?ùâTÊ\°?°å%´¢"?¯9±$P@º?Ú
¢ñ@
'Å—j¿êŠˆ_	¥Æ¿´#7èy¦Š¿Ô$«°óRs¿Ðpeƒ<Šö¿Ü¡ººÑw¬¿Í_9÷GŸ§AGNbll3FGL J0710.3+59081H 0658+595?ïö—LÀôv?EáØãÚF?"Zo'Þsø?#ՖÅo"?P†‹»E	?DQÑùâ¾H?勤w	öþ?"f_³EO?Fé[«…?V©Ý-??"q§Çˆs?'îøÿ%w?ïhŽâAø?…·ÃU®¾?côZ6TI?RyÊx顚?›tbÜöö¬?…X¹ŸT·¼?ï k¬GD?zµ,·>?hO‹x›b˜?TÃ`Ùä?˜è˜ýC«(?yS-Æ£"4FGL J0710.8-3851?ÕÐ:k.ÅÀ*E{cM­2À9œFp&ىÀ;æ~AN~é@õ£	ÚÊ@ž¥·µ?·ûRò[²?ÆRüýA@"ô%×*@²§|0R-¿á•ú=H_ë¿àƛÞÚ¿çöó<¿ê;3¢™Èi¿çʃÁd¿Êëï½<¶ëAGNfsrqAT20G J071043-385037?ïç
oóò?[Ú._µ"Õ?QP¹u·BÏ?I͙ß0ږ?`JƒÕ0jS?Uœ{ušm?ï»qhj4?…$:÷Þlš?6؃­Êì?GÈÎ>K?€láÌäĤ?"¼"ô/¦Š?î˜îÏp D?Ž¼áaï?Ò +Á—°?wÙi|¾äê?¡üŠþ•Ê?ˆ]P?ï?æa-À?ΎßÃR?k|Vbêp‰?Y6纪%?""©
ê®Û?[ñð`ç4FGL J0710.9+4733?ï½ÿ$Á^@6Ìt§qÉqÀ9ýçÆ²À<Owï$æi@¸Ä(äOË@ë꺝 ?»ËA1xö?Ãv.^b@*6âëC@y	³ˆB?ï!#}´¿æY*Fy¿è¿ÔáïÛ¿çq·20Ô´¿ð?ïÿÙi"A'AGNbll3FGL J0710.5+4732S4 0707+47?ï÷ÿ½ÎgG?Vdt`—ì?FFCX{Ûû?P¢Bo#?3uŠÛΫ??¹žƒ˜æ?ïbÛQŒj?"ó|Ægfã?i"íús±?ƒCr³ÉÆ?"qpÀd?ŽrbÁ;ßð?îÙIÙÐ#?‰!¬ÛûËÂ?€dO¡Í¨?yKkåj|Ó?œÈ+<õÍ?'é	~âFM?ïŸlTv¬?s˜˜¾_Å^?s‡¯,=*c?cå–Í\"?|Â&˜lÌ­?k™Gcª74FGL J0712.4+5724¿äR±íg:æ@9ZakTãÀ;s\,PÀãÀ<µîj¬FE@"(évј?ü-­$ß³?ÎRœ-Q?¯ÅHŸ5Û?ã?Ðà@ÿ'¸ÿ»b¿ç£æߝ‰é¿áÅâÝÛ<ý¿ïš@2 ?æÿOÁ^Y¨¿Õºt»=Ù)¿ÝÁ'œzIAGNbllRX J0712.3+5719?ïy'k'ä?‰p™ø¨›?:̕ÿcâþ?5ÍhcÜ?oàC Sþ?‰$•êî"Ý?ï²Ôβ0s?'·OP¼å?:RMmN	?Kî6ùÍr?'yéÁxõ?¬{‡-Ќ?í¶.±¦??–%÷dâ¥+?ie"Ì´?asÓþ¾!?±†s‡I·¢?•ÚàZ¡Tb?ïK¯¾ëû?>ñ/ϛß?S
ên³Oâ?WjsxvéS?›eÛa7K|?ŒÆ¸×‰Ã
4FGL J0712.5+3311¿ãéą38Å@2Žª:э&À;€y1DFÀ<¤ªIë@ #÷êï]?ÚI…ÚõÚb?ôj\_|gZ?îûÀÖ…&?ó¿hæsg@˜'°H1ȿ畟¿MˆI¿é¸;Ÿé¿îÍD¡š™õ?éÚFsBî¿æPÊï¿ïú'`åóåAGNbcuNVSS J071224+330953?î]¯á²dš?­Nž*®Ö?~–mþZD?ƒbÓ@,µ?¦R4CYë"?«–]ft[A?îΰû®V?±ZÃ?Îe´É"´?£¿4´½Ê™?B­¯×ÊÓ?¥-¶®Ñ"î?ì[‡Èâ?¤^À !?¡bm›6?œ¬—áÚÄ?»Ë&Y+f?¢ßøMœ¡?îÏ3«Sûû?¢¬¾Šeg	?·bë}Gž?3r¹¢Ù?£é™J¸?¢¬‰ÆfŸ4FGL J0712.7+5033¿ïZúXÁ@7Ý÷¯îpÀ9ʉ%®À<9M÷×ü@Oô**¡@wڎVo?¤)#~¤?š<&]#?ón_ċµ«@®B"ùF¨?ïÿH˒:¿Þ±	!ç±U¿ä)S€°"ˆ¿ã¥Ž/L¿ã{A–£E¿Øºùe²€AGNbll3FGL J0712.6+5033GB6 J0712+5033?ï×#‰3¯?oΞYU¸?&ÑãÆìÖ?#a Ø1?sÃ_.É?o
¦Û°¤?ï¼÷ï¬Ë?`â¦ÊYÄ?>5츻\­?Qó×¼l"? ©^lä€?}HßõI2?ï«×E™?"ßOïI	+?nïóÆ%¡Ö?`â×0ÌÄ?œ†ž™xƒ?ƒRä£P?ïÞ©èMu?YöVˆ¹?P~úèŸ8
?>ýCÞÝ©?iñ£bîÙ?UÑî·ZA4FGL J0713.0+5738¿Üd…ˆë@9wt¼j~úÀ:ª‹#À<[AE÷@sáo@Î@Ãa	/T?µ±¿?Æi†?µóãqT?þ! v˜Ò@úÿý{ÁA?íjAQÙçh¿â•?í«À¿åÒ<öˆˆ¿ã£š8ûÊ¿éf\፿ïȶ`x'AGNbcuGB6 J0713+5738?ï¡1CÏ?ƒ%üvŠ?U	äøހy?H)âæª?…ÿüd?€æ	[wôm?ïÂ;Ë…?}íܺ@¦?=pâT€W?TMW¸–#?}a\Võ™?{~ù¾Œlë?ï%Ûr‹®R?¦‡,"ÄÇ?p7HUF®?`óY?—6¿™8ŠW?~ý‡¤EøL?ïÛލz!
?YÏt6$*a?Jø`Æô?8jÐ9@?mcZT[øK?W«6Ía¦…4FGL J0713.5+2537¿ïÉÄgu@/Ù¾ôœõoÀ:¹×†d2¯À<ƒÅg}¾@¦¾p=«?ýǝÓ[\?Ðú±AV¥?Ò—ÀÑkî@Ÿ¿ž ß?üë&¢E?ïÿHµ{wp¿¹ò4æ;´¿å±æÍ)¿Õð9Õó<¿í¡Š~ɉ¡¿ïçôpÄÜAGNbcuNVSS J071336+254016?êÐvÍá4¬?¹
r—>?ƒÇ/¥Ko1?{èÜðýŒ?Á±Î&v[?¸µpÄÃ?è')œM²?Äeã#"?°	ýqˆä'?±ÎqO|¸€?ÅòZÖk&?ÀßY!5¢?é腟ÍÔ?¦{·ûZ?¬·@êã\Â?–Û'°5Ý?Á0Iñ? Ò«ÚÎ3l?æó`?§}¡;ƒ†?´9ßÏ<?¢ŒTfá²?ÊÏþáÊ0?£"1qé+'4FGL J0713.8+1935¿î¹ü>ïê@+'ãÑÌÀ8Ü#™b<5À;ØߑËnÿ@_""	"@-ÍbôÁÞ?ª";}üÒp?»	7¡¬ãx@™ûçl‹D@µˆMÁÔÌ?'%f ‡¨¿áˆÿ΁ٿå4ƒ•KV@¿åãÃb(¿ìçù¸¢ž¿ïúÈRꈟAGNfsrq3FGL J0713.9+1933MG2 J071354+1934?ïWÓåVØ5?¦˜€5ój˜?iØ'°?h/TR™g?'â $éèÿ?¦'pÞ)?ï±mJ¿?‹ƒñ?"ªo?AžK=?]i›2ð?'ŠËŽx¦»?Š½Y¿'?î\‰Ø©ºh?"$IŠà?ŽOuJ6;?"ØÖ0¡Fš?¡ð:º¿>K?Œ¸ê³r?ïñÒڗ!4?Kæøe<"î?%©àõkݘ?4âU;J?Y¥³­?J =F±Z4FGL J0714.4+1110¿Ò"@`º¢J@$H÷‡‹zÀ:Èû>ÐhÀ<rŸC@Ùî»4@¤XÍ?ÐÙ=^m"?ÃØáty¥?ö¡]b±¦@|Wt0('?ïýƒÿ("Ÿ¿ÝûÙ)Òa¿ádže0[¿×î,-…tI¿åŽœ`w	¿ïÿý¡UûŠAGNbcuNVSS J071416+110830?í58a§›?°0*T†^?ZƳ u0;?U1SÏòÆ`?µë"$AR…?°×Î4Œ?ê}K³‰)?À¹aíb8?h]ö=a'º?zaȉL?Å©YXæ%?À…ÅtwÈ-?ëbã÷ÛÁ¥?¦Ì¨‹ë`Í?‡™DØÈ?x5Ì
˜a?ÁöŽÌ«à?¥WÀ~ +?îcÓ¬ïtÑ?'{Ú7p2Š?qÎZûÇSÊ?ZÕÆR"SØ?§ˆùяÈm?ºÂ–Ÿöz4FGL J0715.3-6828¿ïÿxô(uÀ6øƒ‡ß\òÀ;i•ÅσÀ<xÉ7Ã@šh®ëƒ@môݍq?Ä<Dÿ¹^0¿œsY>	Ðä?Ø#"Øå@.`÷炱?蝷€µG?ÊOø{QZ¿é¥b$¸F-¿áÖ3ž$E¿âešŽŒ^¿Ð~Dß-!¡AGNbcuPMN J0715-6829?ߓJ›? >«‹')?h´Z.ÌN?amWTú?£Ò†Á(i'?Ÿ~s¦ðòŒ?ï:%*(E?"Kº¦âþ?Tÿé"ã'À?cý'›J¢?—k\#l¾A?'$6'0Óá?í`ié´WÞ?•INûÑWµ?€O׉ø?qŠfIûÀö?²ùÆ·l3?"¦[þ•?î;ô*rÆC?‹˜¬«R?q<õi?É?cnŒ l…;?ª«¯ÓÕ?‹GF»nš4FGL J0715.6-4528?äþi°{fÀ.
_V§¬'À:.ÄBº³À<S"}¨¢K@ïE…pB@=Uæ¼b?¶šõº¿rdœBÞz^?¸"~!™ï@wNö³%1?ïõÄr‹7׿äãü":µ¿ä‡.]
¿åÓPÊï¿ëüœ#·•?Ûáad°AGNbll3FGL J0716.0-4525SUMSS J071544-453031?î$©¿ÌEy?¤Ä{•Ç?x"Vja!?r/Ñ¿î?ª¢á8n\X?£–¿ZޅE?ï~Ð<T&?SáÍ9ûT?GïP½ý…?U'º˜p;?ŽÌøÕꙞ?ŽDïÉÌm?í6õ¹M—V?šì©´æ÷?"Ráfè­?ˆ±h³9e?±3™ÛóK)?"êYÊ[Æ?ïôDÚ?~A¾(ðá?v[=½
{µ?aÛ(ÌëRÛ?—•r!^\?zÍZzݝ¼4FGL J0717.7-5519¿èÁl¶%…9À2zîÇÉWÍÀ:õÈ	ïmÀ<ŸµV¬µ@ úÿ£8Ô³?÷´º6È*?ÒÉu)wȎ?ÞÁS<=@âݽµØ•@·a·?Ôúß?ï]'îY¿äÎ˪Þ?µn˜K»À¿álN']‹¿êÜUÁR›-AGNbcu1RXS J071745.4-552024?îqSz×7? $Ü á?'·ŽVk›6?ŽUÒ%—T?Ÿÿú9}Ï?˜ߋ—=5?ì퓐Š®R?º'5½´)?—íI𥫀?«p!®ë'»?²˜ÿ""?´x7<?ìS à#u?¡<;}?šj`¸¼¿?‡|©m´ß?¸ŒŒ`е/?D
 úì?è†3tz¤ñ?°a@=r`?«oo›s"`?¢'ö²Âi½?ÇVG8‡f?¬É—‹µœk4FGL J0718.0+4536¿éêOy1f¢@7tàP7PÀ9ÃJZ—%KÀ<G'ñ·gá@Ls 3&@û¥»ç?²°Õ_îR.?Ì-˜ªwŽ@o1'Y4@*€='(?ãRâ/àm¿Ò]³ß@¿ç4~!nÑ¿ç ÐàWÄ¿í ìt2¿ïúöv'"AGNfsrqS4 0714+45?íZ"hÇý?§¬e~7O?®‡L~¶Þ_?¢‰ý{?—­yC?"8f½'å?ïkß»ºo4?Ú;ÉL†?`֏Áƒð?n¢}Z_?i6Ž)$?Ž>M'ŽYs?ê­@§oáu?«Ié^ñŽ?´ÂwB'w?¡§ÁEY!ž?µÓßM>bÝ?¢:ü…>)?ïh"¼‡+?wÍSNûu?yKþ®ª?gˆ•iTh?‰KjÞáîÝ?qÅAȪf4FGL J0718.6-4319¿ìÓÁZu8ßÀ+OíA·ZuÀ8œT§!A™À;'³ k°@ß¥ídó?ü¨J¡äÁ¶?¤Ÿ¨@?O?¸‡žß–ä@€€B_@´ jÓ?Õá¼'-@¿Õòâu«}È¿Ý÷:Ÿ
Kî¿ÕÚJ¤>
W¿âŽÌ¡ƒÈÍ¿çÈ}GS{¨AGNbll3FGL J0718.7-4319PMN J0718-4319?ꐧ?fÒ?µZP–e)á?âS´øé³?¨t¸úÔÔ?á‹Åš|?´-¨œA£?ëÕ^‰Ù2?ÀºR]<)Ó?¬	ª"Ý.«?¸©U|ÓÂ4?³P6ŸÇØP?³ç;G4&?æ«<åÍ;?°Ý(Ò<®‹?²göYf ?Ÿ£Öbý÷c?Ì>ἃ?¬ÔZ¶•?ä/÷"^úK?°3™dÿؽ?¯4_>³9Õ?–ÚŠ0ÊV?Ó¹…Ók¤/?²[ÛÌÛ:4FGL J0719.1-7055?ìèLÒcÀ7R™ú©vÀ;Ø©yámÀ<£Vh•ì@ '—)§Ä?ýá¥Ãsˆ?Ìý™ô2ld?ÊáYv¾Î1?ý§Ww¶@`õÏûUv¿Æ¯h¸P?ïÛ }-¨? 2=ûõ?™¿Úoø æ¿ç;Mlš]¿Îyz?a>ßAGNbcu1RXS J071910.3-705411?¦ó²?®ržü?hWªïG9?b» s["£?‰‡ë‡A«`?|‹ =ªä?ïð#w
Ç?•åÁœ?d7øÔ-³?p¦ð@óL?š'Áq?"Dd)^¥?î±™Ìn?Î
ӍA¥?|5
T9-?n/¿nN?«^L‹ßr?»«+4î ?ígrBÙ?'‡`à½?"o:% Ñ?´=Hk?°­ä¡?nø·‰¿.4FGL J0719.3+3307¿îzl¡O+È@3Ü£}™‰À8‡Á*[À;§Ü®ÂË@1<¢ô@¨l›3͍?œRiH1á¾?ºctïk2S@ 4çhY†@cÇ8ä")?psecÜô¿Ýû÷|ù¥É¿â­½½æ*¿ä0Ž]{[@¿çTèÅP׉¿ë`B5ÃAGNfsrq3FGL J0719.3+3307B2 0716+33?ïœÐIèÊÅ?€¸à¸Fç2?W'EK4Î!?Ugê+ø?…ÙÄÜfµ?Þåàd?ïA3¥8z¯?š¬ÀøBìÝ?eOLû1¬?t¦>zL>?•/©ïQD?™MÖ«P?îåò‹Cªõ?"´Âtd²@?‹¦]hcXÙ?‰þøÀe7i?•nãXôþ?‹Ïvu…Vö?ïÈ!ñB*?j܍~?P48ߏݙ?Eúï§!Ñ,?wáùAúô"?g¨z	¼íÞ4FGL J0719.7-4012?æ×$ˆ9dÀ(VȒ«hÏÀ9¾Ò–³5À<ºö
³¸@–R½<6@x+h{?¶é±4v?®ò«â$*Š?öê¹aµý}?÷HýLœeÒ?ëG†Â&€¿ãr
™E¶Ã¿äÑ[ý¬¾¿ß ϧƿäퟫ+'U¿êi>]ˆÇAGNbll3FGL J0720.0-40101RXS J071939.2-401153?íêî‰Üb?ŸSD ÑÄ?yÓ9¢'ñ7?oßáO.™g?®°-ç:?Æû»ÊÐ`?çK­ñs|^?ȁu!¤f? ; ¥л?¡¦ÙMnÊ?΀ñš\?È
&PH
?ë¢aåo ƒ?Ÿj¸ÏeH?•<~ê?'\›á?½Ñÿ\#?œ)æ«ù?ææ÷=ÿ1?¤{ÉrØz,?»‡`Õ^f?›KòU¡?Ƥ¸X´‹? ØkAz?4FGL J0720.0-3507¿çþã%ÇÀ#ÈîñºÂßÀ: žóu®À;ýPMö-@ѯJ/ùî@økú$ì?½	§ž•?ˆ1È=à¥?ËnÞÅr»^@©èsFs­¿À"dÌ2s¿äK G2Äx¿éïa|¼¿äž{`sˆ8¿à'ª&¯—2¿Úk	Cº[AGNbcuAT20G J071959-350448?î×ÕÈiV?›Q<HËõ£?W"aßÞÅ?R[¬x&F?¡Æjl{?š¶ËÄEôö?îeǗd‹)?°†¼ðÁýF?'gÁ¿?Cóç,;[P?©ŒȪŽp?°€ÌÀ+J?í¾ö¨ì"0?—"Ñåš?}§æû½?nj""fv?°6€GLîÌ?•Ö–vÚ»?ï¼&žË2¢?d÷0S‡à?-]÷oXX;?›³Eö:?€€àouõÑ?d¯˜•Þ"4FGL J0720.0-6237¿íZâPäìKÀ4¹"åûqüÀ:1SÃÌsÀ<40i@µ—;ÆU@¼›"Ud¶?ÇWèߧðÊ?Ï5E‡Á?ý5Y~ —@›èñƁY?îó‰p"¨¿èyÂÅâοí5#ÞV¿ìÌJ@•òE¿ïÿv}_Ò#¿åÅ2à'AGNbcuPMN J0719-6218?ï¿#Zr^~?£·¤îsä?s¹Â)?¢î½9üu?jÙ2	ee3?q€ö'‰8?îÒÄ9i?°a—oï¨?‹¢¡ç›»º?™?ÒPnÒ»?§º6¹Õzs?¨ÿºš)W?ìòMDž8?¡Ûš"=Û?'Íx9Ðɜ?‡Óp7»¿?³º7Ñ~ÛÚ?ž *lM¶À?îy¤#äå ?Œ^;×P?'¸ÕÏéç?·©qª©¢?žn­"qè?'.¼iéN4FGL J0721.3-0222?¿ê
¢#	@2Üû:À:ØúåäËÇÀ<b7£Û;û@!
ÂFá'?þ-î \+z?Æÿt>ì$?mWtárÏ?"VdnÆ@[Ž(¢5Ÿ?æþåþ÷í7¿îÏ
)N­ã?ØâõãÇe/¿åQ¯õüpÿ¿Ø©`Ó)ˆ¿À°{±|9AGNbll3FGL J0721.5-02211RXS J072114.5-022047?ãÈè"(Î?Æc_Ž©¸?d¨P¥.S?[³†2±Û?ØDß?¶d
?ÆUz'7<å?ä$e¤??ɐ" ™×?oTñóÞT?ÔDߎŸE?×x‹üÏÅ4?ÉEG_ù?èÇÖÖ
`¹?¦´¢yÈf?ˆûd¡¢9?pÁVm;¡Ì?ËPî]¼Y~?¥õ·3ð8?íN Ç‡?—=µH©d?`v:9û+Â?V6,›,"?µµ)©êt?—ö½—ì¥4FGL J0721.3+0405?â×3€`°@!.3ïñ•À8îH[¹d:À;Ö@&t@™`ùj½@}ÝÙdŠÄ?­Ù=ôWUQ?ÀtƮЍ@u–AöD•@à‹†"¿Å.ld'5¥¿äÊf¿ç5ם‹@»¿çÿ©-‹S†¿í¡#›æzô¿ïÿç<t%AGNfsrq3FGL J0721.4+0404PMN J0721+0406?ï)Ɖz_÷?´n~•´N?M'èÊ<(?¡bb¼œ?' eÜNã4?«/ŽóV¿?îñ$»ÕŒæ?¥ê¼83c?aFQÕAó?qÕ0¿_?Ÿ²žJªºü?¥oVÕk?î}ù‹™¤?¶çO¦Ô?‡S²~]¼_?~µâISï?¢Kz®žö­?Š>™¸†Œ+?ï`¥ö¼šj?w%ºž&?{²vÓ·
?gā³Ó	û?ŠL©o‰ß?pÊèEú­4FGL J0721.9+7120?롆¬SP@<»à~íÀ6CÀ:Ð{?;2@e°Ñn?ÿÇ@ÿ¤?'AçÅ?­ÄÑ<w•@"¿U›=È@§6ÀÁ&¿¹.CŠCeZ¿Û3ÀîÈ¿âJ'Û¿à£W±—½¿å›aðµà¿ä1Ÿµ<OAGNBLL3FGL J0721.9+7120S5 0716+71?³#óM?€¸­¶iU?QIr§ö†®?Q:`ruV?‡v$â\?€¼4(nM?îã"?–Ò@?¥?âØ/òÉ?w?¹œŠn?Ž+í"WÆ?½©Ë~•v?¡»ª'¸Øj?îW¿EH3¨?ÜPlŠÌ?ŠKMt¥õæ?ˆÑ¾<5†?£ñ8NSH
?™&S'7¶?ïÛ:wÉô¦?e=7!õ$_?H"È(ÿ2?Gx05Â9F?n½Ä>?c`Á÷ờ4FGL J0722.7+3606?ïð×uÆE@5ZÀ?öÀ:¤p¼*¾À<xåÈFUO@æ‡ÒǸ'@ـõ]åŽ?Åã!wôÙ0?¸ÔÈnÄ-í?ðdåÈFUO@º8	0Ö?ï—ùá­Ún¿Þ—¥ãÿÄF¿é¿8ÇǪ¿á)Œ 4Rî¿ïý
í™Ëï¿àIí>²B]AGNbcuMG2 J072255+3606?ﯨµ«ü?€-—dåC?a®î1P™?_ï§tÍ?T'Œõ°?}—…"ò?ïG ™óò?'šXåþf?fÐôEë†?xŠ)—E£?"AÎ8ÄJü?Œ°V@?íðÜHtÍñ?'×î°2&Ô?†»'»?uüÒðêÄ?«q·3<?K`%:F?îÞâ÷v>E?pú¸.«?d
À£†?uÞ¨Cs©?•qš0æ·!?tó'±Ïð4FGL J0723.0-0732¿ïSò"äVŠ@_9K{)À9äٞlg1À<±KgŸ@,­†¶h@°››ÒXþ?ºu…NQ?¡£0P¾^?èÍm¦Ìˆ@º	Å{ ?ï‰>½ªðÚ¿á{0f…p¿åÅ$aß¿áKñpD¿àÈ.3ïò¿Ù¬¾Å"3‡AGNbll3FGL J0723.2-07281RXS J072259.5-073131?æÚ´v'àK?µG'ñ?ˆ-hà˜"Ô?xoý‡5B?щ+Ì«zË?´á_¾Æ§Õ?ã0Nd-?Èº¬gj?|£ߞ1ª?†åÀÃÀýÖ?Ù,Ö¿¹-?Ç˲«m̀?çû¤R=—i?¨\\ñnÕñ?šÇ1'—¹?€vÉâŒZ?̸ˆ"Ç/f?¦¥pþ'?ê&ñ¦m$?œáHÊ{`?"
Üñ§?w²Ë|\×Ñ?Å}ȹý?›Á"ÖŽ\4FGL J0723.4+5841?ÛÙi=[U;@:ÿyB=À;å¼i¨:FÀ=¾@Bo@"{é~^TÊ?í@*ýڋÒ?àfQÒ[?æÝñLÞÕä@È¡#і`@a«ã=?ïÿõÿ 1#¿ç²›"nÝ-¿ïÿÝÀåãÊ?ïý¸Ý¬˜û¿ÁSIÔ	'¿Ø=ª]yAGNbllRX J0723.2+5841?î¥>Øãó?¨¦ã]hi?zrÎVÿŒ?zû®Þ{?¢]¸¾Fàí?¦‰pHÙ_Ÿ?î¥#•ÁÛ3?®Tì¾?vŸ4
?Kíö'À?¢Ùã ÛËD?ª±˜›vãG?ìHŒ6GÝ	?¡iýc ?´—JŸ^?3lúУã?¹Å:×ÃÑ?ŸÙe
±ôî?îãޅãÜ?£º]tPS¢?kàŽ5?‹þê5ü?­s¹7r?¢§Þìclˆ4FGL J0723.5+2900?â
lÿ@3AƒÆÉ}À:¡4êÃWÙÀ<h"»@}¾ýVW{@iüp?Ð#þA¹Þ³?ÁfbÍT²?ñk:á}^@
¤ý·PcÆ?îáßeUÅ¿ãô®ÞOV*¿ãôC¾ñ—Ý¿ê~è=k›Z¿ïõÉ{´Ú¿ïþI¡ßŽEAGNfsrq3FGL J0724.1+2857GB6 J0723+2859?ïêôïcÇÉ?a3'$³?8,ðOÍ ?4èS+ss?br'UÝÑ?`Nà	e©«?ï"Z†Z€Ê?ŒOºÊ¶S?T\¼1|Í?tdž°.^?ˆhÒÑٝ±?‰e©?À?î‹Å!§–?‹ÂÅè…
?zõóÁ©NŸ?p¹"è6'?£äïmQtí?ˆ·¥TÝzö?金ÐCèn?kzØðÑl?]Ö´üâÍ?KöåÚß?ƒ"uOi‹1?i7Å|¤:ð4FGL J0723.7+2050¿ì@½È«ˆ@07!-w1À:Zڀêv+À<c" ³Ô®@ £ˆ6šÆÀ?ÿkªs±?¹*Â÷6ð¿¡xô2—Vô?ç:ê _@ü°­\o¿ä›?î¿åôi"PY¿âA¥¼½‹¿ÙɱÅ	‰ì¿ãêÿ½ºá?sKç¢ËAGNbll3FGL J0723.7+2050GB6 J0723+2051?ï_Dp­Lf?e@œ¶V?bX¤¾n?`–S†֕?'Ì]R"E˜?Š\…GˆS?îëð¨éâ?¡.."vý†?_u$9Æk?g€Úa	Š? JwÓ£.Š? §Yêì ?íÐ̃3?"-[e!—?{Ï84û?höKÀC="?¯"$å(9?'Àâ¦í9-?ìüÖ~Á¡?—ââý"?y…§¯?mP+ÎW¨?¶!º¯˜~?˜
5kì4FGL J0725.2+1425¿ë"àD±á@+Ó"Àh¡À7ÝàÇU•À;‰¢TS>k@4#.XX@ —Œ™?—ÄCøc®?°²œøž¸@AbÙ,@¬¸ú²ä¿Å"V¼OQ¿áfÕÂ>ÔQ¿äËj—MŽÿ¿ä
оsæe(]í!¿íƒá¡p'°AGNFSRQ3FGL J0725.2+14254C +14.23?ï{ÄÅ2ÑY?ƒ€°Ü???DCNóÎù?<ØÕC?Íz~\l»?ƒYwê½mQ?ï¢f55²?JÃAj1?O¤Ú}Œ1ó?fÌH'1é?…l0ÊÙÐh?"ä\ÆâG?ïFõè‹;?…¢½³Ô°¶?vʗÃí?uš–¾Iÿ+?'n
‡?€Y-B9L?ïú"%·?;ñ"¤õ?î¡·q‰?ÜjË.3;?FÅÃ÷0¬?:øqÜøí4FGL J0725.5+0216?ØÄÅ䝛S@!AlÅûø4À9Ò¹
x)À<ñü1>f@
Â
|?ÿ1³¡'œ'?ºÇð-"£?³¡ö4z0?úqºÝ¶ÿÜ@ÑîøEÌh¿àã£=‡J¿Æ(G‡S¿ßøÔ<­°R¿áAn?"՘¿Ü/0Åпæ%Pò`ÛAGNbcuNVSS J072534+021645?íµBX?§Ãjñ²D¨?fZk¨°–?bbhÜQ?±7‡Šúm?§2*4™!Ñ?íŽ
ÚÕÖ?µ\´Ã†?SX¤J©qŽ?iû'¨8?³BF˜,{y?µS¶?íRVÅ°ÂG?˜:i¡)?{¡9V¸à4?lø$݄¶‰?³³6=_Ç?—$Îõ
?îšUR;¦?Ø!P¨U?pBB´¿ýð?VÔ€âÏ8?¤VÒTDEÔ?¤`¬MȖ4FGL J0725.5-0504?½ ˆK=–@í:>À/0À:Û_D35·À<BxÔ'4!@!THÈpǓ?ÿ¯®(œ×<?Ãs…]Íf¿Ÿ¯¹|Ê?ßÿ^¢Í @aW<|Þ?ïõub'¬¿ár"›R×=¿ë*:э%î¿Ò¹'"µí¿åµ(€Ò£P?™òåæ#`AGNbcuNVSS J072529-050338?âÁÒëҗ?Ã#ÞjŒÁ¡?n¾y£[†?`iUÀ(Mi?Ú>ÝþÏ?Ã&ŒGßAª?ÛIO¯sͬ?Å¿h×ǚ ?†¨¿Æ'äJ?'ýüv?âµ)+͚?ŗâ—±ç?èiKX""?§Ú~&DÊ]?Š´@¹Ò'W?r~콯PÙ?̯Ž"Ú¤É?¦Æ`+ò¤?æԂeI²w?®Hj"Ì?•eWŠ£,?‰'/×Z÷?Ñ¥¼ÂhP?¯pº6Í4FGL J0725.6-3530¿ïª>°tÎÀ"gn¤"ŠÀ:Åõ´L£GÀ<!6ãÁÛØ@ 0Î"oO@Ãlß&k¥?Äí&ο ÏÉ£Äã?à'qßÁ@Fx	|?ê'ݝ'A¿èæT]Of¿êýÑb]ÿ΁¼ÙÏ|¿à'8¾né¿à:Ã_æš~AGNbcu3FGL J0725.8-3532NVSS J072547-353039?è*œ§$?ÁØAŠÄÆ?q»Rnyþ?m(Æfê|è?Î̪ÏûØ?Á¼%#ì‡?áõÐȎNë?ȋxw<
?RÒµNô?e¿Œþƈ½?ÜXœË¬Ü?Ȁ°Šîãû?êÞÞ³N?¤ë¶ð%?gks§«?p¢t–?ÃnçíøK?¤òiÿ ?ì÷‡1Ï?š
‹ÃÅ+?bay©LL?TËÚrC·?·°º¤9¤Ì?škWÂf"4FGL J0725.8-0054¿ã&w9-¯L@ñµ ÝDÀ9@†ºŸ¤À;ûbqåª@k¶ÓfD@£ì¤©(?©¡ÛÝ`î­¿"Fù¨fÕ¼?ê':…7@–¢n5é¿áaÂÈg¿áµ2Ùà¿âíp3Sê¿ÜŠÛ»¨N¿á%_Ö)lá¿Ý×_¢ÒÓLAGNbcu3FGL J0725.8-0054PKS 0723-008?í)ríNƒ?¨à¹¨rÛû?_¼-çGw?Rb¸h­€å?¶8Û°øn	?¨°…۝ö?풲XWÜ?´{¨o`'?O±L/ðQ?e	l
<2?³+
¦ý`ß?´YÀ}lßH?í[íaÏÜ?šý| dÎ?|<|?j|Æ|Ÿí?³\×3i¿Ð?™‹ÑÃOx?îú]¯ló?ƒhg–•¹2?p¢ºiÚ¨?W8ï¯Ö?œ…¥¯›à?ó>½}¹C4FGL J0726.1+8114?æ––b‹@<ÊÙ­…àÀ;çè:ç\›À=#Èb±@!r˜k?ûkëšî-?Ô)|»'gÌ?Äseè½O?ð<÷ØQì@‹cöÊw¿ïÿÿ)@k*?ïÿˆ¬Œ%?¬,©ßÀx¿Ú"s,G†§¿éôœßõ¤?ވ^Þ²¨^AGNbcuWN B0716.0+8119?ïH±ðn¨C?—ÂÈ
þ‰?bÛxE9œa?^"ú¿æ÷¸?"ŽRéƒÃ×?—6²(ÈQ?ï2å*Ò«?–±RÚ¶Ž?`Ž¤ÉQ¢?púš<—?šGÎÈì€^?"|_îˆn?íTøÇ;¢?–K²úƒ-?‹¬ðøY?ƒ€µR²ª?±â¡0f?"$­…^h?î´mµ]Ül?Žv¬ãV¢?z¦Í."¦?qßöÞq¢|?¡dK
fÈ?'4Ú¬¥N4FGL J0726.4-4727¿Çú"«uå
À,J ÊæBÀÀ9$ü!N.aÀ;ÂÁÀ)P[@T!¾@Âé@?Ä;-Ó?°s‡Ù~?¿úš ¹D@@a~ @Xj1Ϳ΋ÜÁ¸r¿ä•¤ýzꂿåÍùƸ¿çŏc}(¿ë—à±Ü¿ïÿÿ" 5•AGNfsrq3FGL J0726.6-4727PMN J0726-4728?ïڈ†›<'?eÎ^ºC<?PÙYS>ìÌ?NӜî?m
Ì»$?b7wˆ"tž?識Ãm?ƒÕà{%½X?=}hü{9?\}wW?‰·?|ÔGÇ灮?ƒ0ß%Nå?îð0&ÔÂ?†' Ôœx??˗î.¨ë?uRQ<hrS?™ùsÿ™½™?€çÞÂo?ïQÔ¼eÕ?x•æR{ݹ?h^mâV[Q?T¸F}Ìo?'¹š·z?vöüs]R4FGL J0727.1+3734?ڟåtIº@6Êÿ:Þ"`À;Á­!5Ú­À<é°¤xí@!À?ÒþÀ?×fxÚÝ0È?èùäÝå£Þ?ïûÙ_'F—@~†T@wUCÿ3Q¿ë?.Ö­ ¿ë¹‹§i¿Ð'4è¿ÙcÍÚ¾Òä?¾°»Ê²¿ïÿýFKêAGNbllSDSS J072659.51+373423.0?íiΣ4Á…?¹(é
"/à?‰ÂÃÂg?z`ඪ?±Òá°?¸pC`¥ö?ívÀ'Äì¼?¼۝·'?†ãè
]Û»?œðeáÓ?±mÀŒÞ¸?¹jë¹ô¹?ëÔtx%¤m?§{¯iNoq?'Äo_¥)?ƒ3Ò,Š3+?¼ë@fé•H?¦RŒX"*?낆ozÐ{?³9*OŠ½®?2(}ä6?BUš<õ?ÁìÑùÕÌ?³:_ÅËÕ4FGL J0727.4+5325?çŽÈw@:²v‰ÊÀ:íâXOLÀ<˜V>Ðö'@'èZÔ@ïd†'V?ÊJàc'†X?ÄO3Cú*Ô?õˀœ?üåàaª¿â Aåþw¿æ½£Ï}5¿çFÓ#(¿æ~'bEo¿ìmå€ø¸ä¿ïÙuQ»´wAGNbcuGB6 J0728+5325?ìuJŠlž¤?³¤Ûi[?›J˜¿ß"é?'kiü6?µƒ|£%Û?¯½¶÷õ]]?íËk´š?§4«_¥Ò?‰]üÿ«"Å?9ÚU³,Œ?¬ñÅ~S´?¡ÈÕùÀ_˜?í0¥ƒ¶w?šîÃÌÑø?"<ˆ¢20p?ƒŒƒ¥5È1?²çX«UÀ(?•?«®{?o?ìþÑߓ?–ÈmSKáK? þ¤róOÛ?‰QKû??¯Iïá?'OœFà+4FGL J0728.0+6735¿êsHìáL@<e#'Õ€À:D6•¾BÆÀ<vî>6œt@38¬nÞZ@ñÈ`2p?¾š%@èc½?«Ÿ!ÃÊ¿?æ†DhÜ
@`«fuªÒ?ïV*
ðƒ‹¿è…H©¼ýL¿ë&àtI}ø¿íecœ‡Š£¿ïÿž{€©ß¿ïÿÿÊPËAGNbcuNVSS J072854+673225?ïéX|\?o\S¹ŒÇ·?XÐQ~k/?jù֔Pð?T¯ÐÿÜ?V|´T5Q?î0†ü+Lü?®AMÝìUD?ˆyfƬR? NMZ)¸?¦Ù6‹ÊÅ.?¢·	TN@?íÊ:jà?•rÛD¶òç?‹ƒëMר?#Îk¥<?¬~á†I@?uº܎‰?íðoÅÈz?—$!'?¥¢zSqð?"øœq,¹ê?–­¹.
?¡e"ãúì4FGL J0728.2+4827?ïòQs»
³@9Òe8hýÀ:´w
}—À< ÝÆT@Ÿ1ƒZ¾@'Ê<ϔ'?Ã;äI·¯?±êÄÚe?î5r£‹‹@yþô'9¿âwÉЙ
(¿æÂ
÷9‡á¿ÜZ›âŸ¿ä &æô–?¿ãø?"û'¿ïô ÞÇÌAGNbll3FGL J0728.0+4828GB6 J0727+4827?ï•Úòð?êÁˆï£?Z	'tçØd?Q"*>,)i?‡HEÔ§/?~F"kñœ?ïk@Î?ŠúÏë'™?Q4£R³Ð?\Sm_@œƒ?'‰ÛíÇÚÏ?‰f¬uMj?íÿ÷o7Q?'­IhŽ=?ƒåi²â_>?yIùYì?«.ŸÒWá?f®Ð	?îƚW¶Ó?ƒC}'jP?yR|Մ÷-?eé>jÆâ? l_Óóè?'Ç"áD9K4FGL J0728.5+6128¿Ô0w@;ûd¾ÆyÌÀ:b]¶ŠkÀ<üýíI@%DĀ"$@\»‡*+?Ãe4b2O3?Ä´ú<ü¶?ýR;×F£R?ÿ®B0èU¿àtéa#q¿áÌ{n5gÁ¿éޠ4¿é'Öt{'¿ïï{ÎRß¿è!^™HAGNbcuGB6 J0729+6129?îÇü6‡?˜ˆ—{eÖ?ŽÔî©Ê¡Î?Ž{£$4F^?—–J~3?Æ
òYQ?êûñPpbê?¼£¯`VÀ+?­E¡S€?°éN78Ä?¹˜R«ÓYë?°ÐÜÐch?ìi"Ÿ·œ?0Á1¨?ÛyJÛx?)/£ZÐ?µ<ý(K€D?•AMÜ¢ x?ëåÏño½…?¡Ê?jwã'?³<RӕüL?›4$==èÉ?«*[AØ/?ú)Grù4FGL J0729.1-3131?ïðѱôÀ<¹½üOqÀ:CTY©À<Wۉ(2@RG[^JŽ@À'¢Ü?ɸàœ7ƒ¥?¾JÍْ-?ðEUDÖ@JSÆP±É¿æ-z¿âp Ñò&¿æQøàüڇ¿ÝÝç;ãÛÝ¿ïþ¸Ø#B$?ïזàÜAGNbcu3FGL J0729.5-3127NVSS J072922-313128?깤S}-?¸|°¢jζ?ìÍÌ£Ãð?€ÔÑl§Û?Ãú¡ÕAk?·Åé$Þÿ7?ä¨L¹1Ï\?É­š|8?kµ¯GÑÿt?x¢.Ôã(?Öwû/½I?Ɂ˜ŸvJ‡?æ{衞ë³?«ÄV:Ö©?¥]St†È?‹|e~'¡?Ð\"Y³—Á?¨à¤f=ðm?헴x/g>?—zÎw:%?zHš÷<
?kžtëìúÐ?±™W´ÕRI?–<£ÞØŸ4FGL J0729.1+5703¿ïì|™ÈWa@;'ýq?À:¶nÒE²'À<—…\˲ñ@V±<£@ƒ¥An?ĝ•½ ~?¸Ø›ž<Òª?ñvÙ*© ö@ïéW•?ï¼ÊUú˜¿ÑÛiþKtó¿ê=7˜ól¿ßJ(B>hñ¿í­ÞA¿=¿ïø#'¬?AGNfsrqTXS 0724+571?ᅥÔÕÊ@?d1š3ö?Z¹?á@êG?TÌþ¤²†ã?yŽEœÊ¥?€ÍLت_?Ðø?ˆ_g#(?N;…íà"?^wÄo¼?ˆ0D»|d?…ù¯Îiœ¶?îœH¯q	5?ŒÍ|çë?ë;I¦¨?v«Íș#(?¢>
Ÿº©'?‡ÇO|	?ï€u5?èp?q9&lðf°?rþ)F…Zw?^×¼‹OyV?†cžÃ6þ?k—æ]ZìŸ4FGL J0730.1+6852¿å*ÆR4U@<¢5¤À;ôrKvö×À=x,æ0@`ú'ùÄ'@6âÔv?Ö&DÉ^?íâþ1ɦ¨@u-fj˜$@~=F\…½¿ï÷Ìàméh?ì¦-['Ý•?ÏÝê@ûó¬¿äîÝ}I,¿ïe©!ÌÙb¿ðAGNbcuNVSS J072949+685305?㕳G³£?Ën†‡··!?ÊqÊTH?ÂϘ¯œA7?Ç7h­+)?ÉPÐ43?Ú¥R‡ÿ^ð?Î&äVž†?ÜÉü£M?Ðt
QÊÈ?³Æöº!†?¶ÈkÈÂ6?⣘ÒfÍW?²'-kȖ¶?Ëaó ¨hÕ?¯1tyé?Ê©•¼aÍ?§šê•4›_?×7åÀ0?º/&ÅÛ?â´ü/P?ºôW*òä?ªñܤüâ?Oo¸7¡¡4FGL J0730.3-1141¿jfMfQ@	ì:P]æÀ6ÂôÐ÷Ô¸À:ïø»h {@ÓÑ3¹ÀÖ@ ŽÉ[ÿ?ŒS¹Vç?·5Ed8@'€2¹¯æ@ç÷¤'Å:¿¾>Ž;Ô¿àñKÞ'ñ¿äÞDÄU/¿ä"BO/èü¿è=N	xNÆ¿ë÷ãœ*ÙAGNfsrq3FGL J0730.2-1141PKS 0727-11?í•ï%›v¶?£~}¿±0?e®ïÀr?eS@T9(Õ?²£Zü$N?£'YŠÕ©?ìLüY9•ú?Æ[¶Eús›?‰;à!b†? 9UH1Æ?ºp¡2ÿf?Å«²rüU.?íŸ`ýî'X?¡ÊN%?"^ÈøÏôY?ŽdnŽÅx?«Ú‹¤®ðD?œI"9iÉ_?ï*:§ˆ~?oD^{á?uOª»=à?r"¯þº÷?•dÀ`è?‹[T—¼ìC4FGL J0730.4+3308¿ëë0CÙbv@6NÆ6°–À:D¿Z'ÈÀ<mÆ	d-@æu27}?ýˆßØBKÕ?ÀA«›úœê?½T›bÇuu?ýƒ«kS51?ü8ÀA¤¿ï{œŽ@ ?ïñ¾>¶ì¿Ý!_€îýÏ¿Ô É°·¿ä´êÓ¿åÀ_–¾sAGNbll3FGL J0730.5+33071RXS J073026.0+330727?ï‡9û€?'>ä"Û?cuò}Ę?`&—0 4?‰k¾Dšn?ûϕ*T?ð'?§Ô^Æâ*?ŽNîmn;?–iÃ)ó&r?§1µ¤ÿ? Ù…vúX?í®LXp[À?'øÂNÍF?"u'¯-ôœ?u˜æêöû›?¯ýÖ
.ÆÕ?RZ.Ö³Z?ê±q9ÍßÉ?ž€|ÜÝü?¯ÍpéÜÊú?'mÞôÖB?º½¼¢œ7?—ßG}Sõ4FGL J0730.5-0535¿é"¡]:÷@Xr)é–À9C_V§¬'À;û[Ð
nï@Oªú•@(šE'É?±ŸÑÛÄ?°ë	_
´@~%ŸÌ¹'@º'
ÛÑ"?ïîè¶7_¿ãDêJŒM¿ãI"â s¨¿à{ÿõï¿èiýà)¿ã,+6åo[AGNbll3FGL J0730.5-0537TXS 0728-054?îÂ\Ʌ¾?—%ƒC @?_'Še…:?Ëî¼4Âp?¢à÷û7í?•"8iœs?íx®49É?¶]'Ûw[À?Z¯)Kðd?jÚr用>?³Ò_ŸQù?¶:C°
/Å?íГ¨wY?'ôàüŸª
?|d%ɞif?gÐm7"?¯j@¿[ý#?'¢Or-ƒ?î֓ì¤:Œ?'q†¥
»¿?}Ü@4/<?c$š¸Æú>?¶r^lÊi?€¨ƒ'ÔÁ4FGL J0730.7-6602?ÚàtSŸÀ4ËݵR]À:(›)¼'ìÀ<Q7Âäì~@!>{ßI| ?û†×¥mã2?¸ûŽ^I·?§¯rÉÌf?ð$ύqm+@ó…'P¥¿ïäY`Äeö?ê$õî.Fd¿©7q@Ñƿޛ0þ$³"¿ÙXÜ¥‡äe¿Íóÿ*AGNbll3FGL J0730.5-6606PMN J0730-6602?ïˆBõX¦?…é/]n?Qw~D#Ù?IlÒ+?‹À@Qã?"øÄCÈÞ?ïŸlö¢Ãù?†ÙüâhÕ¬?=qtœh4l?PŸŸ´t´?‡96²kÀ9?†Ø9Úý?ída~¾,¿?˜M'b?~Ô}»V!?pzÍ_ä??²ï¬.Y9
?–Œø…¸ù?î<(G®8º?ŠòPv­Ô?x£ï†mÀ?gKo-¸c?©(ý"N¼F?ŠüIב4FGL J0731.2-1403¿éÚþ>gwf@–ù%ñ+QÀ:*Ógñ€áÀ;ʎo™ëÏ@ûL¶çÞ @/<c]j?п$ÃÍÕ?׈'=Y@·kcü(Û?ø›{HË Ó?âñn!›±!¿éçÇßþù¿Ü$ýŠ·¿ÞŠ0]¿î1ВT*ú¿ïùžrAGNbcuPMN J0731-1402?·S¤Êŕ?©êœ­}?¸UF&0?´NKVoü?êªâ¡äç?¸à~‹P¨?º°g©-~N?½ytåùÉQ?Â|(Ï"?Â\
šœ?è
érÜQ?ǃBðž?ÔÞÎ÷u?«§Ä–c¹?˔"Ã?©ãÙÍ7?ÝWèeI?«ʝº»`?¼KµäZ0¾?–Ô?)O6?Ç'‹,ÿ"œ?¬á÷! (?欦x4ØÁ?­Æ©õpB4FGL J0731.8-3009?äuÙy¿šÆÀ–4T›bÇÀ:nb
·'À<'‰±Å@ n·Ã¦3@ʸ¥Î[B?ÃÝ
Ý~ Å?ÉÞ
¼×?Î*ÚÊ"Ý@åàÄüI¿å˪Þe{…¿ä¡L`«¼\¿Ø^ìŸ{¿èZa_ìNÈ¿Éŕ 
;¨¿è,¾|¨AGNbcu3FGL J0731.8-3010NVSS J073151-301058?äëØPI?ÁÌçÊu?qñ°z»>y?fîñÞ(j?Õâ!6drt?ÁÁÔK.'?åe^6
'?Å|º`Ï%?P¦ÇA~I?j‹Lûó¾f?Õ$RÊ~?Å^ƒè²×??è'‰«é??©ZÙÌ#bÔ?'}j…ÒL?{/ÓUUc^?˧䈖Ù?§´Z
²#€?íÏ\™N1?'ý¯ˆXQ?Uÿ€Ë|)?M\ÔùæU?±/‡Ê?'Wé €¡4FGL J0731.9+2805¿ë:pÊ@4¦£ßm¹AÀ;3x‰|ìÀ<·v Í|@ M«¤?þ{Ê`áÂ?Ю†ü#»?¼'îY?ìH^sRÝó@`¨܅ý¿ÕIÈ`u¿ë!ªªcy¿×ÖRß¾¿Óòó¨é¿âÒ;66ó²¿ïÿä¼­šØAGNbllRGB J0731+280?ïªތÊ?'™èúð$G?Mn¤ëŸný?V>ø/º?ƒ¡ÞDÖ?€©
®§=?ï¼%m2?"ö2×%R§?XÊøG€à?b@;QtJ?›ËÍèö{?"4°á.—?î!ò4ùø}?ß¶q¤¬?tˆ	°4h?a³³ÇÌ3?«^¯*qº?‹ã¡÷*¯¶?íþ ê`?ŒÏª¥>EŒ?hñ•…n@ã?Xkg7ı?®†Ý™	Û?Œ_î@"9ì4FGL J0732.7-4638?·sr/]ÀÄÀ)«"«CIÀ9ù±ñ\ÏÀ;·×Ñã@"ñ>q)ä@Õí6´È?ğUÆ0%?ß±Þ¿"~M@9½ÆŸŒ"@oÆÚðQ?ÙÉÉã
€ò¿Þ—$'¯À¿çXàÚö±¿íÞ[€px¿ïûE@Pýô¿ðAGNbcu3FGL J0732.2-4638PKS 0731-465?î]]ölB?¯FƟ®"?›hv)ôJÞ?¢ZJ×½V‹?˜ë˃u? »ÓgÜ£?í» Ñwø?±¸ÿ[ìÒî?"NõB§×?¢Æ\ÏJ~?ªžxG|,
?«'ã)7?ä°6"¥˜g?°_¾Ù*lq?ÅÞ¯{&u?¨Uìë\ú:?Ç`vrC'ð?©ß׏
ý"?é|X'ã2»?§ö¶…Òíº?žx÷P×?‡ß'‡
C_?Æ?‰2?¦e@Èôbt4FGL J0733.0+4915?琣ý(gÜ@:ÄÝ?á—_À;Ž"çƒ1xÀ<ÇÓØZ@ PÊwGà@¬Á¾¢h?ΐä>X€J?¦ƒÝ‰wQ?×ì$ÁUuR@ƒ,,®´´?ïÉ÷šÖ°{¿í',ˆG¿Ò–ñH­ü¿è]b
â¿×óµÄÈqs¿ß¤L%šAGNbcuTXS 0729+493?î+Tå­V»?¢ž/%…?`¶XÿÿlI?\€/ÓÿÏ?¬?L*˜?¢"ÀÓ¡?î™@jɞ?£'ö4"qX?pa‡†…ˆ?9"¨ŽÑÖ?¤iS˜b•…?¡–4i}ª?íhÛÅ_Œq?™]'%?{"̉ûÈ?l*Û³7ÉL?³Õcßù?—±ÞFd¸x?î'ȋÑ?•F(€-ì‹?f@ÿö†?`eƒñ¬È?­¼#?³Š?•žPŒ	
B4FGL J0733.1+5910?æëª)xŽ @<KªX-¾À:¾åžTê=À<¼:ìe‰@£³1fª@Ûä—Å?‰Å!Ý ?½Ý¨<I²Q?ö-íy¾Ô?þ:|PªC?ï¹Ö…³2È¿à˜›¢ˆU¤¿á½Aԋ³¿å^ˆM@û¿è܄›Ó¤¿é ÷IíAGNbcu3FGL J0733.3+5904GB6 J0733+5909?ìÄ
왦Ë?­Á0Ç6u?"̏$PÐ?éy «¢ÿ?´ì"ÒÄn?ª¾Ñ·¹?íÓ"-à?¤\ó'ëb?‡è÷§Æm?ŠéªØÀ*ã?¬ÔX囆¨? ÐØ+:Ùá?í%à8­%ì?—nŒd]?""Aýb.?'M…AAGË?²m»>Dø?'ëGÉL1e?ìSÌì؜?"÷œäb?­ä*¼ÁèÕ?Zµ^ÁÆ?¬ßu´U[?Œºž´£lV4FGL J0733.4+5152¿ìW%%Q/@;PÜY1ÊÀ:œ˜¬3ÐÀ<'·I­Èü@ ëË|Àšå?üWu¸e?¾Ú¡ Ì~H?¤õg £#?éUM9n·@)Òh@Ž¿ë"Š.B¿á՚ }#¿ß½<:¨¿Ô;»P¿ã1Vº ù¿¾™AGNbcu3FGL J0733.5+5153NVSS J073326+515355?ï…l_«?q D\9®$?F©[Ÿ—:±?:í‡ï€¾?{è\~Ã,?po`ÆÙC?ïl¼-^¯?Š^"#CÛÀ?NÓèC¢‹?Xäޜړ…?'qÛ Ç?‰LH¨´º[?î`ßIµÕ?Œ\·¦PXú?qÅJñócx?[G6bƒ?1?§¹bÆ6V?ŠÑ¥T9x†?íõmúóò?'F×Ôá¿Ó?s뵗—î}?bQÒ͇N¹?®+©Íá€?'FÑ㽸Ï4FGL J0733.5-5445¿îz¦Ç!±À0-VJQ]À9àª_ºz»À<M‹^¿@ô¢""EB@?A^o!?·ÐK\tË?±š}Å'¼Ý?ø–ùáØ͌@j¼¨'Zá?ïûbví'¿ãŒdý°šg¿âdøbQÙ¼¿â/! 8B¿ãɵÁŒä¿ì"~w=AGNbcuSUMSS J073334-544544?ïðó繟]?qæÐr9Öï?&]G'Óáu?6óÒ}ªcž?[L‡œfÆÛ?pŠ«Á*ë?ï՞ 6Æ?|'X§Žš?$³8IÇ?>-£zÀՁ?tŒƒ
ÊÛ?{ÛT…Ý+f?ï)Œø¨2?}@Ù¶ÛÌð?jн$Á?c¹ª{$v?—'¶½gâ?yÙÛ
G
?ﴋÞÜ??jÍѦLÅ?JR¤
¸Ü?8æ#ɇ­?4óPHDÁ?iúӓÍHp4FGL J0733.6+3649?ïñ‡—©@7ѾãÕýÎÀ:·óáäŒÀ<'³!*3@x\fˆJ<@°Ò€jôk?ÂÇ·#Ã(´?¨÷ð€ÊÚs?ã:¿ïn¸@
<åc?ï´èâÄ0¿ç+zl­¨D¿áֈ7q†U¿äx#'¬?¿íë¥jˆ4?ÑUÛ}¿žAGNbcuGB6 J0733+3650?ï"u?yxš?ˆ´Åie—?Z%PÕ<?Q"u~ŒÈñ?‹Ÿë}·¾Ä?‡Îٚ°ƒ–?)]A7?‰pp,ó©?Fi¹Äà?Wý'Q‹×&?ˆ1¥=d?ˆÑ-¯`¸?î†ÐdÊð?Ž)´vÑ8?…`†:Ëa
?€Uó	0ÊJ?¢:Ø$«X³?‡áÄzý ?ïOð'Í¡?lcžJz(ÿ?d'ŠõÏ?R›j}¤_^?ƒ‡Ÿ¸#ç?hêÆy '4FGL J0733.7+0205c¿äýÎnQ[+@$º±NÂóÀ:¬i—sN¬À<"/|@5@Í$¶n@è"C ç?ÑúeŒKÓ=?ϗ
Éĕ?÷›bÇuu@š1P/p?ޜJØw{?ïڍ¯ãˆ¿éÔ¿?E-¿äÙÇQbÉ#¿ëä¥Ï2¿ïÿú¡œGtAGNbcu4C +02.20 ?å¥s0^È\?Âz{× z½?¹éѤ…ô?µÖDNÏþ?Ìu¯U²›•?ÀÐ‹]?ëX>NwµŸ?À·?m‰?•pß|¥? rf:o?¿øqTcQ?¾û¼8)Æ?æ±	ÊVÙ?¬¥¿óG É?³…/9¥Q?™eÄ4"?ËwlU¹Ñö?§ ð ÊŒ?ꠏ‰^ÔÂ?¡{°Q™0?¥V ò©ÓV?'o"1w9"?À(9Ú8 ?œEº5:Ô4FGL J0733.7+4110¿Çù2ÆѶ@9
»ìª¸¦À:=~|Ý¡0À<yy1DEª@i%u°[R?þÙ.T§!B?ÀêÄ.˜™¿?ª€câAm?î]eÖômü@ݤ]ÂÓпØC¯AÌ~¿å5f͔s¿áˌ%<Ðk¿Ö®êäâ¿ØãP÷,r¿éUÂ@þAGNbll3FGL J0733.8+4108GB6 J0733+4111?ï8$09þ?‰Ë–þ\gÎ?h©s—<?[/ý»?Ä?•èÍ%ßn?‡¾Ð÷ón?ï}µóÂ|?ˆ}.ßa?M¯d…K§?[LœÔNû?Žàâ,ÇŠ?‡-uŒ°ß?íß\֚?'6ß{A?}$8~'í?jÖ©ƒ¹bv?®jÇÊbTÛ?߬Ö?î|ñ·[ç?ƒÆ•'^ãv?wå9¤Ýl°?b !©ì…?¥;9¯î"ò?'¹LF4FGL J0733.8+0455?îÍh•."­@']—5;À9ÆØôù;ÁÀ<6	'_Á1@O}–®®@ÊZ¤'Da?º8vÿeÑ@?¾V§V›˜!@€ê[Sí@š˜jÅp¸?Å8(%
*¶¿å(Tf,Û¿äP‰OŸz"¿ä`
+Òì¡¿î`~oò¿ïÿâ~9ì¶AGNfsrqGB6 J0733+0456?ïËë¼ðc?}Ô'±‰‡?R‹ÒÉ»þ"?SëxzE?ug,ՃÏM?z`9¨~­‰?ï±wd¦v?ˆs˜þ7z??Ž×^ùB³?Z©»ã
?'¥Åkޘs?‡¿í~Àbm?î³zƒÞ¡?ŠÑ‹'³G?ƒrg'.wÚ?{×S?x"p?Ÿ×{Ïö?"ѸG9m'?ïÚôþÙ¨?ZQ[ÙcZY?NS¯è$n@?<$–_ú?mv,ä<Û?W£È7Ø4FGL J0734.0+5021¿ÕÙÒç¬@;$"ƒ‡ß]À9áj'"À<gœâ#v'@ðy©åE@&ÜB‹•Ë?·ëp&É?Ä¥"¹¾R@5\FR@Àx¿¯Wò?ïÑ>¶ôô3¿×þT.U}á¿ç6òl¬Ò¿çÆžEÑ¿èX.•>Á¿ãò,"à`AGNfsrq3FGL J0733.8+5021TXS 0730+504?ïV?"B;e?ŽoōVm?r¹@}þ?j4"©[ñ3?‰»óèsÎ?ŠƒÚøýy?)`ê?ˆvÈòjN?RƒF:Å1?aû» Ói?Œ\e>þ!0?†‹¤±› ?ñ'J?Œjn÷Á†?Sâ¸xd?u¦íCb‡È? Àî=@Ë?‡ÙÀ™¶"?ïr­‹U	?rØz¯ÌÁ?|‡¼|?d<{?ö½?…¿.¡²`?kPx‰¶€,4FGL J0734.4-7711?ïØ\³À8
à"S.À9i)•ûhÀ;ç$¿ÒéG@=@ޗz†@nXæK#?²§òø°€f?¾³k§ÃÓÕ@
í$%y6M@žL[Î2¿áÓ_
+¸¿ßM"ÜIm¿ã¤;é»¿ä ˜%ü¿éã{dû,\¿ïïÏ0T[¢AGNbcu3FGL J0734.3-7709PKS 0736-770?ï덥H`%?XwKô
Er?9ÓRáú9?4"±NT9?a7ðt£œ??Vi=;M—?ïÏë°
‡?{z$Ä?0:èsêÝO?@"ï»å,l?wyv:Ž°?zc,L"t?ïδu«›?‡jAPMMÓ?{Fb3"?tÎþt-+Õ?˜"×ؽÅ`?>ørˆ?ïÊûÜŨü?cë'ÏIã?@֜Rræ?08äbï?xg>Ý%£?b'¶]Ç`4FGL J0737.3-8247?ïIqD¥–À9y¥CñÇXÀ9ڛ<1·À<8¸¤ Ü@ýäG'»¯?þ=þÈs¢?¶_l÷úøÚ?°ö!YìÛ`?ûz4ääÇ@9CiŒ5®¿ï£Ùqö½?ïÿxPsµÚ¿àý|Bם¿ÜS¿ð›^¿ÝĶv$J¿â°ÚÉÒ+AGNbcu3FGL J0737.8-8245SUMSS J073706-824836?ïÕBÇ]P˜?g©·-ã¡?LëmõEìñ?D¯È‹ûÖ?qÁ.'®ö,?dܪ¦ø"?ïU2>×<?"ïàÍl*?[ÒÑï?ic¥†\=?"®€«kœ?'SXï»?í8RÃ&?˜gǪB/?†üÛÃé?z:ýj4x?³]Îo&A?•z
v>æ?íÖ©¥¾?Œ"šÙ‰?'ý'®ÕÅ?8
Ì]¨?©–œX]uG?Š|çù¡4FGL J0738.1+1742?暣<ä›@2÷ß (À7@'§À:ÿ³"ý*c@[‡/‰°m?ÿ¬BÊ ?˜wñ†É?®îŸ&÷@Ý­àx{<@Õ r'B?É	¤C–­¬¿Ô<rwá¿á;ã:Í[h¿ßJål[¿âÔOb"Èõ¿ãY™~Á¦ÿAGNbll3FGL J0738.1+1741PKS 0735+17?ïÉ¥RDŸÏ?yû´ä%ñ¶?QÒòð‰i?UòmOJ_?v¸š!ªv?v3%¦?îîò¢CâM?Ÿ–Ù,Õ?u³,«ã/?'ÛÔ!}?œ´àŒŠê¼?â!'n?íª2žnŸ?¦—üKGÉ?'—fB0æ?À¥ì/;?³tìQ{þÇ?¤wýÎÁ?ít¯ÀÏI?›)ø靱 ?‰²3Òw?u9ùÄÖM?³æ{6Ð?š/75z{4FGL J0738.4+1539¿íê2X—Ʊ@1O\žf‡ôÀ;mÄ@6PõÀ<½Üºí§@ °€¡¦‰?øT¨Ù ˜?Ø̙¡&V?âØ\î 0@t¤Ú¦@UîcöIž¿ïÄà\+¥?ٙiþX5?îŒÖ!à$˜¿Ò×ɓ\i¿æŽÏŒ0û¿ÖÃT¦Ë±AGNbcuNVSS J073824+153839?îân³º©¿?ž¸Sև.á?ƒ¡¬SƒJÞ?":õ$¾¬‡?™áS^é"s?˜²MÖ餷?îPtºs!ä?ªtþgIgC?Öά`…?¿}«6?§~øU©?¦Vàç«Ô(?ì˜G~>l? >ÆC!±u?'ïã€ý?'ÃIƒ`²à?¶'K-Í.?œKí"K6•?ì®]C8q"?¡ˆþS±°?´
Âp!?x³ÌsúG?¸Zÿdä%e?¡j7Þf?4FGL J0739.2+0137¿ïE	Õ6º@&Á,I4&xÀ7')yv
£À;tcŠ	@¡œvmŀ@'>3Av?"[M¿·¡©?¸T=ë.H@ "¥Ξ@Wˆ"MÞ¿ÏòUk`K¿â³¼ÅîŒ:¿æL¢:Rf¿æ‰Ã}˜²¿ëÌ>1"÷¿æüÇ0«™vAGNfsrq3FGL J0739.4+0137PKS 0736+01?ïKBÕáÞJ?‹ww'Js«?gƒPþ°£?d]—ôR¡?"§;#î5ß?‰Á€ùÂKý?ï[ʕ'Ã?šA'óŒé·?n¬E~»NF?…ýŠå¹
ô?Êýx=ò?–|»A–ÌÀ?î~³1­ø?—Y
 R*Ó?"*&?uÏ3?Œ/ÝE)Øp?œÿsŠË-J?Š:Và3?ïæ|<FPž?^±W-6Ð[?B™)yg´?<ÖÔ®m½?dÝy[hp?[äÁ‹X˜)4FGL J0739.7+1743?ãÃ×ìÌ®@2qWÿ›V2À:˜)W_À;mÓÐÍŽ@å4`t	@ôZDïô?ÊÀDÔt?²ëJç.ù?ï+üÞ@âaFkõ¿Û0³¼…à¿éË4çhY†¿éôàM/¿Ý´áÙú2¿èìЮÝ*¿ïùÏdVÁ®AGNbcuNVSS J073948+174304?îZ(À?¤ÿîQ;"?sÓ6x¦mÄ?r%MäÒæø?§ã/2A?£Ì´÷
:G?ï
80øZ?—^uÍé4?gÊëRÿ
ø?vÝ©xôY?™$ûl?"òxòøl…?éG'¯cîÆ?­Ý©>WÆ?š4~¿†C?Šóc‰'¢?Ç¡:²˜T?«œvüÊÓ?éÄ~¼aL?§֘¾<>??eßfôô?nޑ\Ýñd?ÇÚ°…+'?¦Ò tÃý4FGL J0739.8-6722¿î!܋ܗ›À4nÑáÃôÀ:døÄ¢[àÀ<[~ùc@ñØSŸ@ޝ"ÐÜý?µx…ø§ñ÷¿µ€°®ˆ"?ÿÜazn['@_"ØaV¿äw6b'œO¿åHþaur¿â÷<b|¿ã9wÑ¿ßØB·4µ¿áWß_¡{:AGNbcu1RXS J073928.1-672147?ïÑÀÝþä4?s¯êyzý?K''¼Ú?JœŸ³çàÅ?s­>¼öe?qiái'/?ï«ïSñžÉ?"¥`jÆ?2& øiö?B *ª1Rv?"rõûÕá?"UÞß?ï~¿Q"B?……
¥ð?f‡¯þ<5?V¡þ¼º?›Ÿ23°?"í~Í1y?ïFš³/³?{ÆÁKÕj?S¬žøxã?D¹t¦á‹?•ûж?{
Ê˺w4FGL J0740.0-0753?êNÏ¿Ý@EàqÅ?:À:†_-À<ê°¢¦@µÏ‰?¯B@µj£	#?Ĕˆ7Çl'?¥ìã¼à?ß¿½WÓ|@P`ö:¿á
B[Ûs¿Ýbyýr-¿é±	ÝÏS¿é"ÛÈ¿í;'ô:Ïà?ã0} g(®AGNbcuPMN J0739-0747?ç)'Bº¡Ð?Àâ<r{??…eT%'ƒe?|n%àgþø?ѲÙa€E?ÀÅþî'h0?ë
Ò|H8?ÄiVÉÜØI?k—'iý?€äf»öÒá?Ã\¯²Ö'?Ä1 ËAü?ë-ZNÐê?££Kåĉ÷?"zçͶ‰?€ýmËgåú?ÀÛ9ÎLe†?¡º¥L†?ï󵊃ß?FU"xv´?eº±ÃþšÒ?UíVL®¸?™j3/°¯?€>ánÂi>4FGL J0740.4+7300¿èm*2X—Ç@=l" ٔ[À:¼³ÑSDKÀ<;&Ö-Ÿ@}EÐïœ@
«£|qk?"f7.¢¿Å±KgŸV@øpž2@×´³Pz¿³·†
¢¿í^ܙÉjB¿éͽ"¨™¿À'Á¦Ss¿ìû2Ál"¿ïÿí@_Á‡AGNbcuNVSS J074111+725822?ì¢T÷*~Þ?É#ìѼSm?¹Ñ"²Ì*Ø?É8#z<ÿ?q½9=ýãÌ?‡šËgC?îÁKä]?±©ê"ªh,?ˆç®¤–m§?¦Ïô\Ɇ?›bÅQ1=¢?¡T£:Ž?îl¡}ð?š¡št'q?€­'ª`Oë?ÙáfïÌ?ª­ëýˆã$?˜zävúM?ï¾K@N¯?¢[–¦Ð9–?• H×	u4?¢¬¦ø?€OہÙiœ?|Æîî¸ë4FGL J0740.9+3203?磴¶¼¦@7Ϋ%(®À:®Ð!#~À<}æðdŠ@;Gxåo@¡ Ï?À<Ndçá¿ ž=ŠØ"?Þ®@dô÷8?÷úÚl1¿ªMìœöÆE¿å77¤±ü¿çÄóºw_³¿ØÒB­)¿ê0Bhv¿ìqýs]ÆAGNbllLEDA 1979979?îK¨,±é0?¡À9¼o"`?‰"¸‹¿"?ÕAÓS£[?¤àv†¾}?Ÿ*'á¬J?î·Ö–(ɽ?Ï'¬Ç.?v—÷Sêñç?'ÈdT	å?¡¯—²öõ?™
+Ãc@?í˜A3­?•°Äæž?¯ŠM{?€Ç™{ªÝ?¯âœ,?'¨­æH¯?íêÉ_Ô¼?"Oõ þ'î?û;Z?‡ÛúéF¿î?©µé:‡?ŒO•u¼'M4FGL J0741.0+3226?Ùðoõíhµ@7òu¸eÀ;̉>؂ãÀ<çH㞠@#/p-ºxa?õ1©u¯¯†?ÙVùvy!?ÔÅ:çÝt?üGZ·ÜzÀ@œ0K¿ï÷û^ۂ?î3;5t¬¿ïÿÿ^ðP`?ïÿþó…õ¿ÔŸÕÖÀ¿ÛÒ݈óAGNbllNVSS J074054+322600?ï‰OÞÊç?…›wê¤Õ)?`«uÑÒ\Ÿ?YåÍòªq?‰*ØÑ¡ ?"ACH;á‡?ïZé3d<?¦Ð»Í/?aÎmª2ó?" Ž5²Xö?'iÞ2!-?¤]…"¤U?í.Qvâ:??›žžŸgM²?ƒ˜ÕìWì?sdj}'?´Y¥£?™9¼åùÄ]?îÁÚÈÖÓÚ?–ä¦þy?lãӚWÀ'?tav­M?¢8íFW?•ÞîjàΓ4FGL J0741.2-5140?쬋›¡~À+Ÿ™€o&)À:oèuŸ¿NÀ;âŒÅuÀv@\ZôÃ6@™çZÌË?ÎÐè:fƒB?ȶUýb–Î?÷—'Ôà˜@±»ÚN¾?à;ÅþÒX}¿ÌÛybí`¿æàÍûü¿ëȬ¬›ÔÝ¿ïÿ$=Çâ?ïû…|¬#	AGNbcuPMN J0740-5137?ï`'?÷?žo%%A¹?z"ÿ¢–b?{‰Dnð¦?—.ïÏ:)?š5ì‹MR?íé¿ÏÓjõ?°%gäé;W?‡Ìeǃº°?"ûÑ~ÚÎ?«péèb?«£`#8?éjD¤@É?©ˆ"ÑèœÞ?¦&O@5&K?'µÉsôÈ?ÄÍ\a³H?¥ 9s?ë{HH%#P?¢:žê:'?"òµÚ³e?Þ+Ek?¾éHS¸«?¡54Ý"Ž4FGL J0741.4-4709¿ëü–r·q`À'zŒûüÀ:
O"'ÉœÀ;üýòÆ@	ýå¶@©EÄ/oY?Àw€bæÕ?¼íÜ
n?ø©¡Ñv@
Q©BO†?ëö@äv¸¿åð×~+©ý¿èF¬â¡ N¿ëä3¡<]¿é¾Îqèz¨?Ú/‰E
¦1AGNfsrqPMN J0741-4709?ï"Ë©Ux?˜'\Ï$§¥?]­ó,!ˆ?XKRh–q?™Ë« ŽÙ?—Õ¹Ë-â?îW`ªj–?«ZWq›Ám?lÙ¸©	+N?}âæù?¨ÂjÈÃâ?©ÅÝÊéî´?î"¨5'T?•Ó­—#$?|®ïFEo·?pÎ/sœa?ª'דäÜÌ?"½Rð2Çã?í³ß7|ô?'ü"Í´wý?€O|zd'J?jà.Êè?°W¸—"q?'s^"¸¾4FGL J0742.1+4902?ï`Ê¿›$Î@<0_¿ƒ8.À;7—Œy À<º%œq»@©†f‹û ?þ¼‡Tów\?Øj×DÁ?Øoâ+XÉ?ÿQßá|‡:@åµ{øI?æZà‹Ær@¿çÞÖÜH¿Ç&£"o8¿æóá^TI-¿ïûü€¿¿ïÿÅþ&ŒAGNfsrqGB6 J0742+4900?ï fïTkE?'€&,R"?h:æh$½p?d•è.Zü?×ŠÛÿŽ?ùk@ìÀª?T'¾Ø?žúËUŽ¨?tôÕgã"?€Fh"•?¢g<"×?šuˆ¿)w?ì%—¨½1?žz°í0Ï?£
Xµñ?iK?§Ë?µL¸;~?—½OcüÇ?íà]g˱ò?•ß隩¡ä?'åÁ÷g`?{}†»ÿ?­@¹‡?"Œœ—Þ\Ö4FGL J0742.6+5443?îykòu™@=øe×Ë.À8tÇåÝ?À;òc`øh\@š{ú!n»@Ê=p£×
?Šˆ¦úw¢?µª@8M@iæ@;Yr@üþËÍsf¿Ã§Íyps¿á¶vÛ)¿åÔþõhø¿ä_bцoñ¿éE¸põ6¿èŸ^ÕxlùAGNfsrq3FGL J0742.6+5444GB6 J0742+5444?ï΃<%º?pL
éîí?W*ЎãyS?P/ÿmkÔù?s1
>4D$?l±‡½P?ï•m߅d?Žø}¯üÎ?J´Âηý?^ʆ}²`"?ˆù;ýÒ;¡?$Ó%æ«?ï]ï©êi?'Ìîv\¹–?p³i`µ‹?k9•,€?0j­ ý?€(T?5òU?ïýXæê"?-­|>ÊNb?ŒM½à/?^'ûáΧ?1§>øæî?+0֗4FGL J0742.9-5242?¤ÒoùuÀ,,©¬6TÀ:ê&yçMÀ;Ó·?œÎ@ÙqÍͨÀ@yÏ.´H?Åkøa%3ì?ӉU^?±@=X «Ó@òÿf}¿ï¯šAµ,?ï֘ȹAÖ¿ë+:¯(w¿ç±_ÞâÎí¿êzÇw"?׆·¿ŸgºAGNbcuPMN J0742-5241?ï1Ü!´8?—"4\?"–&"âçŽ?"ɯ›€s²?t¹VðED?x÷ß÷UJ?îdêPL0?¯×‡a1ð¸?Œ""øE?ž™Ýª'Â?¢'ÊYþñ?¥»>kÆí?èø#'5?ª¿+Ž•?°ˆIhÍ?™ã¢Ò–yØ?ÃÛg°	BÅ?¤mã.|úš?ìÑ7Áà£?›tz;g]?¡ªf=Ä=_?Ž/ƒ£fL‰?°¡Òä??•, øîOg4FGL J0743.0-5622?ÍÿÂ度ÒÀ/G™€o&)À:@NK½m´À<&¯söqâ@p|ЋU@w@GD?Äym>Ç»ì?Ãô¾""¥?úmlP‹3@"¿ÍŠâÈ?ïÍa¢‡Sò¿æ<|óp¥…¿ëDžj䥿åzÁҝÇ&¿çz4y"P¿ïÿþ½à ¿AGNfsrq3FGL J0742.6-5623PMN J0743-5619?ïë/ï¹ù?a¨sÑ-þ?O«Õáuþÿ?U»0Sµ'?Yíµ/Ñã?Rö<ˆkÔ?ï‡ÄgÔ?øBÀéÃ?Pœvì…p?eI¡+Ëe?‹ûbËa:—?ŽEˆT…ï7?î"ËߣÃT?'1­mWv?wŸƒXqL?kžÎûñ5?£ÏQšµ¡ ?¥3h*.?ï*°åŒ©?yXŽêÁÏö?tÐvœ?\¶ç'_k˜?•©¯X
M?v'Ã9•4FGL J0743.1+1713¿Ç;$™<|ˆ@2÷4Ö¡aåÀ:tt "ôÀ<UXª¼Í@îˆv܀@öQo^?À4X6ÍÇt?2¹ˆà?Ò
þ Vâ@"µW¿ìa>‰R¥?î'úC'œý¿ä£< oK½¿à}á,U¿Þ»ÎÍ®¿åëÐ}ÜNËAGNbllTXS 0740+173?ïqdˆz:?€üí²ŒU5?ovk'?c‡G@Ù?‹ã€F'?}T–‰A'o?ï©ðØ|?…M+cê'?Lè$ñ1"?\U&N‹²?ƒï¸4¶Ñ?ƒ|0[.˜¥?íšUsmâ?""æ·³ÙÞ?"[T؁/?s^Ÿkø§?°­Hùü@Ï?'¹ÅvÓ?îאh÷÷?äøŽQŸ?}>£³Ñ±?föʓuâ?¾qxL¨?|BΌŽ­4FGL J0743.3-4912c¿°²F1|I´À(ÌxB0üøÀ:Lâ\
WÀ<	_¨Ý|@®Ê_	Oà@¸E܃#6?Ŗ^%Ð;?À}Ãû
?ùÃk$;?îDæҝ~?íÌ:5…óÊ¿å{¦3Ûϟ¿è!æڕl¿èe¼ÝÁf½¿ã¢©][û©¿Øˆ§ƒè‡AGNbcu1FGL J0742.1-4849cMRC 0741-4900?ë?óà´3·?¶'`½þ±ô?RCY£?‰ìK¡O?Á{Xù–ò?µ5Ãbð,;?ãò°ÚÞ{?ÎۍNð`§?´>|)H¨«?ºÔ(<ų?Ó
ÿ?ðßÒ?ÌøVÄÈB?é´ AƒˆG?©Ãã{´‡?šf÷•?…A}®'?Åâ¾i²þ±?§X‹nw´?Ørˆkå?©Mº|"ù?ÂR ÛÉë?¨'ž9;Wé?Þd'{°d¤?­œö×x0Þ4FGL J0743.6-3805?àÆzX"IVÀNÁ;ŸÀ:A¨@üI'À;Èu2²ô@Ó .^7@¥Q]À¥w?È-Ûõ‰¯?¸[&þWÅu?ñۑ¦†'@__ô²D
¿Ø"€}¾Ç¦¿åOì!%êu¿åUŸ~àÛ¢¿å›û©Y*>¿égõèO	S¿ïü<@øî"AGNbcu3FGL J0744.1-3804PMN J0743-3804?îB{}¤	?£Lå}Uñ?Z.bŅ?P	ªsțï?«
lN²©<?£õî·.?êÊw¾	?ÀĂñ'w?DgވM?Z—áà—x?Ä ÙÐý?À´ /Õj€?ëQ¨x?£âϺQûä?@9CD?{oÛCc?Àë-½Ì9[?¢z¡p®à?î~Ûõªß?ˆéhŽR»?Yø}$$I?E6Ýc®~?§O¾W"pö?ˆþ²4FGL J0744.1+7434¿Ûç˜RFÊ@='MÓØÀ:¾ù¥À<zŒþ€£ÿ@ –€
§Mâ?ÿ ¥&••ÿ?°¾ØmiåÍ¿ ‡ìa×OL?ðÂ0â (@7ÛÜ_;û?ç"5vÚQñ?d*®Ì©î¿åRÀâ]Ø£¿ÝB€Æ¿×1šânõ¿Í]v¾"eAGNbll3FGL J0744.3+7434MS 0737.9+7441?î¼Þ"àF?"ÂÕ²ÇQF?tYjÁ»?h-de•dj?¡¦û)i؉?')ö+ü?ïTAÔñ—X?'u™»`H"?_Ã6ŋ?lô5"Æ?"{'ÿë¸r?Ú›,¾?íw.ø氃?˜¿ê•d+?Êûð?q÷]êí8Ã?²%…?jýç?•úÁ-Ríá?ílÏ I•?"i˧ÈÑ?–ôÖH^W?åª…Ë?­¹"w7c?'ËÒµ«lX4FGL J0744.2-6918?Åø[NŽÀ4ÇR"ÃÀ:'"Nü½À<E[sÄû@סçñÁ@œv"œ;?Ɨ–I­óï?°1,a¡Ÿf?æéHcF v@GÂWþÅ?ïû¬´('¿ÚZ[@B¿äü‹Rûпæå§#Å×æ¿éù>Dß-"¿ïóˆù8e¢AGNbcuPKS 0744-691?íÖ*Zà=U?°+•7\xì?{ÅÈå¡·C?rÐÁ́‰?¯$¡5Gó¯?¯ùGãcp?î÷
Øþu?—ÿ™‡3?`òK"µ½?jB]—Kˆ?ŸuôNzš?•€ë"¡‰?ìÙ¶ü­ö?›Ãý­Îg—?É¼ôè.?€Bѯ‰Ð?µ9XÝVE?—1¥ÒM‡j?íKwß®‡?Œ*äaÖ©?ŽÔêšî¸?t‰¡ßƒF™?±É£¯-ðH?Š©¹	[é
4FGL J0745.4-2447¿âá¡°"\ï¿Ã<
ÍHÏÀ9¼1ˆ8HFÀ;]H2ž¹@¡Ž_S͈@ä4 ½?Ê>{eÒ?֋I?2É@¿)Æ¢ç @û
3\ó¿Ý9ÐÜ&$¿Ù†ðI©—>¿ìè®?Cî¿ê³¸þ¿ð?ï÷$ß³Y^AGNbcuPMN J0745-2451?êbiI@Å?ÀnÙÄVk2?žYM…©K?¡hD,þÿú?«1*J»y?¿'(¾(l?âN(?Æìà?Òýš ?K?q|Ĺ ?©¼\f°!N?ٌŸ8¥Ú¥?Ѿ>ônµ«?Ý;¢Q_>?³~jæÑ?ºO¢™zn‰?›ËMî@C¦?Ü0uBS?²y[§C4±?ç˸)p}?´žbC‡? D–•#°?‹ÖPBpF–?Ì¿ù¶AR	?´"4}ú‡‹4FGL J0746.0-0039?ïð7jFè@'©Çy¦µÀ:¾?A^o!À<4Ÿá²7@4,}·eÝ@ûÙ_'F—?ʵ'ž}¯?‰Ú5b"ÑÙ?»æ'ølŽ?û÷-Uù†¿?ïÎúnƇ8¿ì	XÙµé[¿ì½ªðÙòO¿Í~(¤äÑP¿ïÊÿ'¬˜$¿ïÿ9+
ËAGNfsrqPKS 0743-006?ïÁäþÖ?@Ã4ÄJ?w9ɸço×?~å ó{¬Q?`†‡K?b·úW¡·?ì?äƒvË?Á˜¨ÎNGe?'9Ù#]*?"k+9˜Tu?»¹ Àf¦?ÁÀë°`r?믡jf2? ˜rt´·?š=L™îDê?ŒÔn54
ª?»ó¡†TU2?;ô뮤€?îLª´Ã?–xŠî'?'† Jx9á?Šýí±ZJ?¡û¦–ë?'Ósf2 4FGL J0746.3-0225?KCùÝOìÀ@&a·À9þoï|$>À<-Ý­sk@ fJ%3?ü<`Ÿ±?¼àC÷ü{f?³Á# k…_?ù×ÜEԉ@	VcȧN8¿ï‰\:­Ñ?ïÿñBÍÛ¿ä!¥Õèտϗ¯I.G;¿Õw•ì¼¿ä¾pžM³gAGNbll3FGL J0746.4-02252MASS J07462703-0225492?ïÜKæ¦?m³ÒZ£ýÚ?8¬Ø€þED?6ïHZñ–:?pO?håI"?l+}6f?ï‰}¨/ž?"­:Êy)à?@VµïÌ¥?R€wäN£r?Œ›*•Iì
?"\›Ñ·?îu_»ÿoÆ?'¼ñ¢>?o«D*å›
?\Ññ‰X<?¦¯OýZ©ó?'–=ˆÃ›?ï6Ÿœ§Èo?wÊgw¸u?cI'ÓL?^?QSn¹V¤½?–ÂÚ0j(?vÙç`•Í4FGL J0746.4+2546?ï¤ïjrP@6ފar
À9ºøW•KÀ<Ëùh6J@ó¿qÅj-@ýJ¡!?À2?WÙ°¶?П%ʔä(@	ÌDÑ	@ã$—9#¿ÖSb}£š¿åX&grÕà¿ìÅî Úk¿ìziR©ñ¿íeŠžT~¿ïý@'cAGNfsrq3FGL J0746.4+2540B2 0743+25?ïÜÚÔúý?}º-—?rhȽºb?r
sÐã°?g'"°í"?sÑX!­?ï†^œ<e??s†âQþ?Xwà?k|yw]ª/?‹Yx·mʄ?‰ýuä³í˜?ìb°܏?¥cVԔÌz?ª.~W?š2³WÊ5?²ÊÓ5€Üa?›®ø^Iô¤?ï±¾Rîµ?j‰'9·»?g9m•³a'?UÈG¾0Ž>?{"½ËÌJ?e%éºx 4FGL J0746.5+2730¿Ögníz@7|.º'®›À:f…8¹"ñÀ<ZÛýÂ8@Wxð+̍@2³Ïà?È*2	h?Ï/՛'Ž9?øœ"ê-/ä@
»
±‰ÐN¿ä¿ôa¼2¡¿ÚPfíÖÞ¿ê
d1Xh¿ænd!¿ï­ÞA¿=¿ïã~õ©déAGNfsrqOI 272?îÅ9wà‹?ž#÷A;ŠÞ?xK0÷>¸?x7œoº‡¡? £~Ã…?›Öx'/Ð?ï‡ađêÉ?‰0j<IÓc?TÌî¢(3ê?f¨¿%Œ½Ù?‹ñ@Gc?†"I±c??íC¿"#*?Û{?Få5?—q¤!?ˆDOé‹^Ã?°€þs?–wwC›<?ïbze«Ô?v3GEs"?q‹ÿ‡aÔ?Y'KåWÒ8?ŽØ›fÑZ1?sv€ðXï4FGL J0746.5-0710?ì¤ÍÿŸ)s@! c¾ì9zÀ9ùÓ'é|À;úPA`ó`@µ¤ÝD"/@»;ªÐú?½_ÎÇ£Ã?ÊÛ¨‡É¤@V4êK@ÑâgÞª?¬MI£¦Ò¿â#BzMú¿Üt»(_šš¿àó 
Ì✿éÕùœ8°K¿ïÿÊ ¢¢WAGNbcu3FGL J0746.6-0706PMN J0746-0709?ç%
3|´?¾Ê,·?ÄC"õ²#f?¶N2aØÍñ?¾ÍÂÿӓ?°E펌Ÿ?æ$½c‰?Èz̙•+?ž0šë,Í?¨·G$Ï~«?ÑӄeŠ:?Æí&úÜ!?êž0³7¥?¨ª>·ºÖ?¬6‰h?œŸ—ëz?½Ã5â³¥?  J3=	?賋:cóð?¡3×å,ªÜ?¦â¼öäj?‰GàŘÐ?ÇyQ§2w"?žS-þ5g4FGL J0746.6-4754¿ê€ù`dÕÔÀ&œYyÀ9¾Ó-À;줾Éç@i*»ëS?ÿØIё?«Ý`\¥â?°ºž¡ì#@"8T~Ý@Ö2ÊÁ?íÐH¢†'L¿à‡·ïÅö¿àÂ_
§y¿Ýe¯¼ñv¿àUó‡K¹<¿ä®mє²ªAGNbll3FGL J0746.6-4756PMN J0746-4755?ïG¼,€ Ÿ?"_!'½?Gxðúì"•?Doy+ˆƒl?–L²è‹)?"ù.ŒiÏ?ïŸnH9ð?'¾ìÔ+x'??ç¿^÷'?WîN.1u?‡%ArùÌD?'`«¿n!?î€ó^CŠ?ÅßúA?sPò4ÆC¢?cä™nå?¥"'ƒ'þç?H,0ˆB…?ïvêè?g\ã-ò?kçŒa‹íã?U#defä?›¡ÿ±'%O?€¦¬с(4FGL J0747.2+4529¿æRr0>À@<hpdìé£À;8F:vôSÀ<½Hɝm@–•-NB?ü±'<ÓÅå?ÖÅi–œ?ÒAIvk—(?ýËûf=K»@O_™m¤É?îi* :8?ïÑÞïäÿÉ¿é¬ðžŽ ¿Ã`–‡f¿æ»E»Ëó‰¿ïù!bü$AGNbcuNVSS J074654+453231?ïÍ@ŒrG?€½Û×øG?jþç°²ã»?e'l9–?…Ìõð¶µ!?}~âF^?ïÈo æ³?˜Q4ßÃÄÆ?lvTæ{r?xû¸'ÐQ,?š˜'šFZJ?"¤åõÉÊ?퓔5׶¥?–ùD©i¾?ˆ›ÿÿdJ?y29/Ç5Â?°OÞQU·+?"‰2fÒ>?íXLxvÒ?šŸ6ÍÜ?"` çͬ5?ŒZœÊ¤?°%w:HÞ^?•‹ü8€a4FGL J0747.3-3310¿ïüóIýêÀôÎf*…À8–·$¦À;J®ö"0¬@¦iÿÎÿ@"œî¸°?©cðüh,?zFäÚ¤j?ч-@´8"«ËË¿»ëXÔŸg¿Þ¡MÃqð¿æ¡wI¹L¿áÆy³JE¿åsUb2$?¿ç2¡<ü
AGNbll3FGL J0747.2-3311PKS 0745-330?ï4G¥æf?@Âp,(A?AXŒm]ú€?<lé9"óŽ?˜ìFßÑãk?
ì·Aà?í
âw[i?»²TI»?@RÿXÝvK?i¶"ú?·w:í"iÏ?ºä†Ô~€a?ì+ޗ;DS?£b•2q?ˆ~鯺Ï?{ø=ËÚû?»'..›.?¢¼cÓ× ?ïAä áÖ?''…I m?R£"A©=]?Aç´«ô^Ç?–³J7É1f?˜¢mvR-4FGL J0747.5+0905¿ë&$	–ú@0zÝð,À:|]Îè0À<€ß©HcF@§e3‹rº@
Òä>š?½ëû€]—?¡ôsb€Ü<?æÃx?ô‡—5秿ï±×~¶ß?ïÿ´‰	)¿ân—²8Í¿âL^G³ó¸¿Üü³Ú¸rοÞüR@¿ÊAGNbll3FGL J0747.4+0904RX J0747.3+0905?ïa1TJՔ?:0Âfƒ?b‰Õð¡rz?Z¾Æ©¼ÂÈ?'ˆš¸'c?–µÖe·?íÊeNm~?ªÄ7{'©?"IÛñÖV?íÚÂÐ?®G4¹¢?§jõÇÇ¢?íœù}¶äY?"CÀW}GÊ?‡kèªÏ1?zIª•ÖSŠ?°*¶üî÷?Ò;»·ï0?ëø3 ƒ§?Ÿº?±úP?¨	Ø0‡L?" >úžå?»{R\ãŸ#?šuƒQMÅK4FGL J0747.5-4927?ݵ¡`ý	ÅÀ'ÑÀ¨ÒÁÀ:®rn²À< Ô¿ª¥@`Í p@ÍüŸù/+?ºšÒSÊW}?¦è©C¨Ù?ï˜ûC؜å@0Ûê÷Û¿àæäÀßXÁ¿ãQL=Æ4,¿æՒn,-…¿Þ¥€B/¥_¿ãì ¾üÕ¿éÙRKý."AGNbll3FGL J0747.5-49272MASS J07472476-4926332?íðlXe¾?¨M;Ü{?s'T‹^)e?h¨ôè†?®ˆïè8ò?§™
Ç"?ï –èÓ ?ëòˆßãŸ?G0lh
]?Wo¹'tÜ@?›3¬_¥KN?\Nª¬?융S˜%•? vɐ?ˆ]©'w?t½‹¶9ÓÚ?¸"y?åŽš‰•"?íé'uš¬‡?Œ½¥
Ø?yÝs.%?hO¦éÓ^?­aI‰®S?‹ añµ$4FGL J0748.0-1638¿Ã±zùg×Í@Ù½¥è\À9cÆOJÀ;´tÇR9‰@Ê·ÚwZU@LԁÌô:?¶iqž'óº?ÃnœÊPœ@xq¡šð@f'ÞdNß¿ÇûĜ|¢é¿å#—ŸC|¬¿é–ˆ¢ÑPÀ¿æŒ¹6£*¿îT6ž!¾—¿ïÚ¼i¨:AGNbcu3FGL J0748.0-1639TXS 0745-165?îd¯Mjî? nzÌ??‰ÿç:¤h?‡ä½þr?£5Jo'ný?š³wð•?맲{?À5%©;]?"ð`>ˆ?–»ƒË‹?ÂGÂ1ïüÊ?¿ŠM­@¤?íì
Ò'ßG?"Ö 8?‰[<É q?xbÎ$¦Œõ?ªø|OÃl?'m  ¿å?ì®zô<×?"11˜r?šn£?cfËÅc?´$–ÃàŠ?'9.PA^ó4FGL J0748.3+8511¿êžGœ@<5‹¤
âÀ:´úȈšÀ<"çä€G¹@ ¶–*´Š?ø+®9cÎÜ?ÀOJ*›Š
?Ç
¸À¦@	ßøØK@ó÷ƒ¯¢p¿ïÿñ¢o+1?ïþ©ôZ°P?Î\u éY ¿ÐÐFŸ ¿à†é~3a¬¿×š¤ÆôE¸AGNbcu3FGL J0746.9+8511NVSS J074715+851208?ï¦d¹(Ò?}mk2mÅ»?sF؀eh¯?pEHy§©?y‡&£.
?r3<>Zá?ïdu"v…è?'ºª¤?]F@ÓßÏZ?j˜¿)¼ƒ?'œëcñF,?"¤Lƒþ?í¬cI% •?—˜©î?ul3¿D?‡äÊhA§Ï?¬ÿb?'´SÁ'† ?íƒägü1?–ÃÕ@É^ï?ƒÝM$SÀ?tÿüz®îÖ?±†­3"ÿ?–
•LñÝÕ4FGL J0748.3+4928?ìóGT@=AÿÅGÀ:µbÙéëÂÀ<Žn‰J—@€§i»Ûc@ü&V«Þ?ɝµÝòå?ÀçàúVGà?ö懈õÝg@²ê%MA|?ën0Ê£&á¿åÑ£€ùÊ¿ä¨ßá¿à–Fދ¼¿ï¼F¢{Àk¿ïZü¥Øl=AGNbll3FGL J0748.8+4929NVSS J074837+493040?ïc¶Bƒ?–‰Q&#¸ß?q|ù%Î]?oÐìjé¹±?™^µ(î<?"gÔYÅZÛ?ï{–®ÿ?ŠýÏyVðÇ?XMñ°ž?gn¯&Ê?Ž͜3Ê?‡ü^¬p§?î}êwT­÷?wÚùbÒ?|àwVY{Ã?t•çÙ6~8?¤…IŸéñ?ŠWÜ.mM?îí°*#Á?€U0oב?"»Ã¾"æ?o6ö­4•?—ì1ü=m?{á¦7'6'4FGL J0748.6+2400¿Ð'·Ôî@6»³"ý*cÀ9T²ü(À<+%üéË
@ñ~Ý֊@S·RDÌ?²J¬azŠ?¯JŠ¹'B?÷ëýáAÏ@³a+"?áÓ¦¥ñ–±¿ä& !]ž¿ãÏâÌ'ª¿ã©&4G/i¿å'«_ê¡I¿ïÿþR€ÖTAGNfsrq3FGL J0748.3+2401OI 275?ïêH_	þD?\7[K{½?4Ðo"ê‰?(^¼
"?c#æèo?Zú6­~(?ïÄ!'³ZR?,Ÿ÷NQ?<¯ԑà?Q0'3X?|$zÉ	ÇI?€F¹cnnÜ?ï+v{pÅ?€.£Ì""Ê?oÐO—Øú×?`Ý¡X?–¥=–È"?|"¡yø†?ïÝÔ³^ú÷?YþÁm}S?EæCyþ|?1þ6ΏS?l±»Â…ih?Xh¥èfÉ4FGL J0749.0-3904¿ç¨/¾«ï)À†?¼À:€ø¿™ÞcÀ;üFñ'@ 
=Šzò@+}\L1?È	<¿¤?²¯«~É^®?ícQÞïå?û½Ö½f}c¿ï`À¹n ?ïãÖ3}Ûοçxâ>ùæ¿ßøelkc%¿á}h@[9â¿ç
¢µ¢
ÜAGNbcuNVSS J074915-390336?Þ¦Mæ5{?Áìë"*?rCi0&
?eöŒ¤³ˆ?àˆR:…0(?Á(Š–9F?ؓ*u®Ý?Ä;!†DžO?pU¯‹Ïè[?z,Ó¦œÅz?ã•É­ˆÀ?Ä=ÜÉZ4I?ä¾LÀ邦?®ñ(Ëàm$?ž6ƒA¬e?'q$$O1?ԟþJï?­@´³Gg?æPx'Ùäè?¦ÿZ€Z?@I_tŠ•?‰Ó빸?ы
FTí†?¦$šj~–Ò4FGL J0749.0-2956?æݍ.ÁÿÀ[íœP-?À:…ôÍzÀ;ނ€x`d@!$ÎÏÜKÆ@ŒÝÉtS?ÌÚväãÅ¿v«ÛKÑËË?ªŽ' cµ?øǟñøUg?؝¯]¦#k?Åíxé˶!¿Ü¤·$D
¿æ
š"U•^¿À7œ¨M¿ê¾;Ú¡¡¦AGNbcuNVSS J074913-295658?Ôô^ŠÜ	5?ÃÙ76ÇP°?rèè.¹Ù?lBFl¼b#?å_þê4ˆF?Ãé¥é?юSDÚ ?ÄP·d‰\q?l5'+,h?}HÏg¤?ç à2"?ÄDázôÈ?ãå´ÓN'g?°	¾6éÄ? 	Ø)$ø?…K}úFU?Ö3[T1V"?®=r)?ãiŒ&í?°øPO¨r«?ˆuí%ÞýY?³…Ãó?Ù3}~ƒ-ë?±0°Ãb	ƒ4FGL J0749.2+2314¿ì‰Ùö´…a@6–Κ,fÀ;˜+ÛPÀ<ÖÖ@ ÚêYûsÿ?ÿJ¹t*t?Ä#ÛýA^Å¿"=Ý8ÞKƒ?ÑÚ@þ¢Ý»?úñ¡µòÀ§?í8"ñœî?ÕHÒ¡ø㬿æq®ÞÐ/ƒ¿Üå<hš¿àO×äXÍ¿Ðq‡+ØÌAGNbllRX J0749.2+2313?îԜ½9™?–"¡,[?bæ%Êó´l?XpüÈ?¡‡ÑÏ·3??•ƒèqiOI?í߸TAéZ?­ÿ¯ ½òf?wü'ÀR×!?"õº<6rš?¯õÃ×'?¬`€-ÖCñ?íéjÜÙ6¹?'6}N°û
?z#-7)?gŠ™|4ûu?®'ÍÌůE?ýùŒ¯ë?髒I}o?¤Š{Y¥zq?œåµýÑʲ?ˆÔÖ™X?ŵÓÐð?¥›>s.P4FGL J0749.3+4453¿Œ>åï!O@<¨1zÌNùÀ9ݍƒá¡pÀ<sn]«¬Â@"'Êö@o¡—Zû?µºµ|Ô?À0µS^w@c<æ:\@
щ5ô-º?ïèB©È»Æ¿Ý꣢\
î¿ãÔÖáΑž¿ä†J!aN¤¿è ÈÝ~ö«¿ï÷½ ‡_AGNbcu3FGL J0749.0+4459SDSS J074916.88+445232.1?ﰝ'àWÇ?vÔO°Èt?^§ØX7Ãý?Y"~[Éî¢?€¤<ãz?sY>m`"ý?ïoµZSwÓ?ŽÜåa@º?`dŽH<î?ouy½j7?ˆ#ÇýÏ?ŠiåHnbC?ï4:?'oºuLç?rè°wäx?c_¹·¼Ü?˜'ûtÑt?¼€
<ÅW?ï	×ÈøÙ/?}y©+
kN?‹ƒ–gq™?p{Î`¦?'=E±!O?tsÔ­u˜Y4FGL J0749.4+1058¿á%¶¥ew @1Î=ÁçÀ:*GÒ&©À<J.oL@Xž¸ge@ø¨ê'?¸?W?JÂ?wâ?Âç?ÃÓ8KËÛ@¤©Ü‡ÕÍ¿Ñt
~^)׿ç¼Ä¬lÚõ¿çi'"š\¿Û/[ßyοæÀÒ@Ìú¿åâ,EhAGNbcu3FGL J0749.4+1059TXS 0746+110?î7G
ý8V? QÃ/jê`?t©*I¹?f§&P<uÈ?©ù®›1`?Ÿ‰!ßp?ï‰ì‡k(?ŠÿWuÜ?P="걄?aE½Ô86?‹}+§ã…w?‡ÝW'öõ?í†C#yø¨?—;êðØ1?‡ó€q홫?x·ó]õ?°ÏvÕò‡}?"µÂ$ε?ï}€FF?Ö­{*?yž'ª€§Ó?až½±à`a?—È«L—¨?{À£©Ç4FGL J0749.6+1324?ïŽkbF«@2ÝËݹ"À:űg¸ÏÀ<uTZË'±@·‹òçê?ÿb¡e?õ¹?Ð@gä•ÁH?àsNÁ¯r@v&}BJþ@Sò•í=¿â·îÿQ¯J¿Ý§!ïi¿Òo,Åǿ敏~¤™¿ïûæàõ"׿ãJ½É#ÊàAGNbcu3FGL J0749.5+1320SDSS J074935.95+132156.0?åæ:Œn:·?Át}f¡Å?Ÿ3â/?¹;×$TrY?ÅÇâ>dùñ?ºq͋Cß?æÁz3¦´?Å=ft}Yø?ÂÓI÷Yh(?Àü3À8?Â&Í:dž?´á.6s·?Þ§i²ë"o?´«©Mg­?Ó&ooÏ,Ä?´(K±
jA?ÌdMºŠ}œ?¨ø™Æ\?çä
)Æëè?¨{é9V??´óE¼Œ‰?›;ÌÞmß?Æg]¶
?¤R´úbÍá4FGL J0749.7+7450¿¹öΗÁìä@=éSXl¨ À:ð‹+AÍÀ<³ çTº@ )'_
ž@N~:˜'B?½ÿ ‡	7¿®"ä¼é¼?ïñà'Œ7@ël‡è—.¿á!‡Ջ¿ì·¬ª–¿Íõ:ꌦA¿ä¬©áæ9…¿ÐîqãD"¿ê݃¬8XAGNbllRX J0749.4+7451?î¼d¾s³^?—ªçšBÊ?lÅÚÁ,/?cl*QÿA?¢mVl²6?–Ú&×{»?ïi¤ë·Ä?…k¹Á
Â?H夠á?T=\öÏÎ?'N݈ X?Œ³n£ÂvŽ?íÆAÒd?" F¥û×?zkö o9?p1#ÕgT£?°,ê°bØÜ?'òӕ~èò?îÍe™O:?‹¿Êvª?eP#G³?\3²?¡Ô¤:å…?‹âÇ°šÈ%4FGL J0749.9+1823?ѝÌæV@4ëßÁœ"À:eËΠ¤À<ÑEØQe@w–÷Cï@ÀXeã‹?ÂáðöLÍä?¯5z`Cb?êæEy†Ô›@	7>$þ½
?ïýU–4ŠK¿èž¿=˜¿ß×µž‡êð¿ì0¯?ž%š¿Î?|í'hs¿ïÿÞ˜–dAGNfsrqTXS 0747+185?ï åŒ¼Ú?…Óa¿)"?VöÁ¾Hæ–?V[cÎn…è?"ç¶c‡­?"®º}@³ƒ?ï{D`%ø?Ž{RÆ­Z?RÏå¹õ…ø?h‰½±#¶g?Žßr0·Ñ??Œd-°¤4C?îY¥å<9?""éͤÞ?}VMSÇâã?w™ÆÖ
w?¦ºØƒ@?ŽOi¢ë?W?ïS(Âd?}±ð™ÝVú?QV¥ÚÖ®¸?G .{YÏÉ?"…}`&4?|îÊe]ã4FGL J0750.8+1229?åŽÀžQuz@2¼… ¾Q	À9g¥‡À<E8ï4×@à–ºìûk@äǕU?°Â5o"¢—?³K—ƒñ$@"ºkáÐ@.Ó8¡²?î¡À_@˜¿âDÞ¥gX¿èŸJrÉK¿ãÂð	è·¿ëÌùÆ·à¿Ü¨ÿéåAGNfsrq3FGL J0750.6+1232OI 280?ïÖx6ë?oè¶c,<?U™]OŠL ?L¸&D-		?o.Ù!OÌ?l01Ê,€Œ?ï¾Ø¸©Y?€ùF?Fœ8¿˜$?`P@"©îï?}Àm"³`C?}ÓÔª}v?îè很m?‰Oê}?z6n`­¯¦?r66è
öò?œUÁ°†U?…Hƒ¥Œ?ïÖÕ+_â–?_üyí"?Z¯2·hˆ{?JŠ—œRp?kÓ;Di%§?YܲÎTOB4FGL J0751.0+7908¿ïÜÅW¯á§@=gT~–À:ŽàùÀ<ƒØž'&ß@n"ˆ7Ç?ÿŽÑõ*¹è?¹.fDØw%?ÊOʘ•Â@ m֝0'@t—>u†•?ÈA•Ì…0¿Ê³!€nÅ¿á	}±Ç¿âÌËN¿ëB‰Œ¿çŽd²1@AGNbcu3FGL J0748.5+7910JVAS J0750+7909?î÷"%µ¿?–Ôs6?1@?"À–é28ë?Ž^X†èË?Š¶HÀ+Íy?†™Û ¢Â?îŽ?ƒ"Ìó?G¹ƒÿc`e?Z¸àp?†b"fDq?'<w( «?ê÷Ïɵ̇?ª@à_Ù¡Ž?¸q——>Ù:?¤ã¶3&Œ?¯ŸÔ6%…%?•D_ÊÚJ?ï°k‰Äæj?h½¬wa?_›Í‰ØE=?J·ÇrxÍ<?ãG»¹Ž?e–ß#2ô4FGL J0751.0-5131?ßå,·e~×À(Ç\¢˜FÀ9‹B¾ÁqÀ;µgôÛߏ@ÅûI{@mÆâ¨e?®Ðó"!?ÄrlN'@Dä]ã
&@ØP¹€ë¿Ò7¡¢&°ï¿ÝÌÔ#Ù#¿æ§¾ aŸ¿å`Âl »¿é™QÀg
Ö¿ðAGNbcuPMN J0751-5134?ï¢RžZ:?µóùÖu?s}7¾z´?~jø¸ZÜ?{YÃòÁie?ó‡vÖ?ï̧•tÿX?‡ÔÄRŒY?2}_4]}k?T!> )U?x"_R:|_?‡Um¹Ìó¸?î»zŽŠí?ìћ'h·?†_R.W[?€fª©@¶?a®v³?Š¶ÁKe|*?ïá—3*r?YÎf!¸Ù ?1Ýu¢)Ý?%Ÿð–ÂE?l7C!Hþ?X»VUJ"ž4FGL J0751.4-0421¿æáÛ4Í×@&¨?NÊhÀ:v6¾/À<k;÷'@k•\É¿?ü5g‹)"N?ÐKÚ®?ÑjÇôö·'@£øôõ
?ôr!èÝúr¿ã™µž2µ¿á1†:A¿Ôy_ã•f¿Ùýh
«T­¿ãí˜>¥­#¿ïÿêњ'çAGNbcuPMN J0751-0421?ìhÂ\tÿ?¯Îi4­áZ?}ôw…ÂêÐ?x<AƒŸ2?¹5rtÀ)^?®çò}÷|é?äÑ£™v?Ëh"9f¶ï?­3øéîþ?®´Xfªà?ÒºrE¯Õ#?ÊE~>*¨ª?ê|?o¦ÝI?¤¬{™æÑ6?¢'&«™pV?Žíœ=NÂ^?Ájx–~.Ã?¡Y#ë£1I?ãÊ]JHÆe?«n5߆?Ä?¨ËÏÒ6ÅU?'O3Wj7?ÕQËq'š?©ÃH‹êW÷4FGL J0751.4+2655?ã\TD®c^@8Tòù‡@À;fØ9¦ëÀ<ÍcЉð¯@; Ákš®?þ'¨¸]ª?ÔÙÄ❙ƒ?ہ¬]@¢Ý@Õ™Qu>@¾ù:!E¿ÕêÔà«"?Î9íwYo?¦dƒ7W…¿àÏûÀÖ…¿æ¨Zý|˜¿ïûC½Äò
AGNbcuMG2 J075139+2657?ïTgœ*§?!˜#—"	?rµ~-±?l¶24
‹ô?ÅÕ¬ïcô?Œ@m£0"»?ï,€À®ò?˜|?¶'´Œ?fIGVn?v—2¤LÕ?—¦¾ÿz U?•"ÒwsÇ×?íq"Œˆí?—Àd¾=g‹?'"vSÚ·§?ƒÙ4ò?°>
±?"L¨'ûk?î±t.Žš??…âèÉþMP?{
µá–?h›=÷?¡‡ZôÉ9?"§%;¼àŒ4FGL J0752.2+3313?ÕÝ]Y³‹Ä@:lʁ˜ñÔÀ8÷tü+_)À<O²ÅºŠ@ùãÏrÄn@xô›Gïƒ?§-€Ä$v?¾}p@é@ˆIDíoÛ@ |ò–?¬9¥=;ʱ¿â?"À´W¿æFñ¡B…a¿æ"ύd¿ì@9
ãˆÑ¿å›«–òAGNfsrqOI 380?ï½¹öGI?œüæý«~?ë"®œ£?ÄM÷LùÀ?–'·j5Èq?šxBÅh§"?ï´?ò"Œ?ˆÜ‰ÁÙ¤ù?FwMb'¤?YaŽihž¬?ˆÈ-8£/?ˆ»Œ¯ê?îi¨2Å¡?š!µŒýË~?ˆÕÀӀÛü?ƒ»`Ÿˆ?£0·ónð?—U"'Q×?ïý»ÊFs&?%p"Ð ?×Ã̒>ýËk睕?/A¥§Ú"5?#73lÉKß4FGL J0752.3-1631¿áÜ©†*@«Oag#%À9ÕVÅßrÂÀ< szK@ #@vè•?þ&ƒøG¥?¼ºD^ÿ"Ë?Á̈ĵ&=@ucߣi&?ú"®LˆÅ?ï…þ|rAf?äl{‰
Z\¿Ú,̼±¡£¿Õ»m߁…Q¿æÎ[}Õ¿×*Šbo
ûAGNbcu3FGL J0752.6-1629NVSS J075223-163340?åeQѯ?¹"¸£?œ¦OÕþ€ó?"Oœd¿F?Ók`^ü¹æ?¹±¬_43?Éþ•F š?ÁžBpYð?Æ£""§…$?Åìc¶]¦?ã×uò"v?Ç^°9IŠc?萚¡JÉ?¥¾HO¤ïA?œRgEÈ2F?†Ù:Ë¥?Ê3H'Š'?£ye\M?àQ܄Ýòü?«çQ§›vY?ÍcD°¡$t?¨äñ;H-?Ъ¤ó‡Ï?§e$¬‡›4FGL J0753.0+5353?å˜T&%j@>8Go*ZÀ9
Ó	ý¯ÄÀ<:wÓv4:@åø˃K¤@±Èd?¥*.B؏?©× –V!@ÕY;¸Ì@o¥åW]4?í¿ÂWþė¿Ü³_=}9¿â¶2÷¤ì¿ß‡¼Aº4š¿æ¸¸
"'r¿â}i[
AGNbll3FGL J0753.1+53534C +54.15?î*iµNX?¡'&I?r'{Ÿƒ?gÆvq¤ß?«vÁ8¾?¡ ¡û,ç?íõŠù€L?³×ï¹aäØ?"Ú ‹îQb?ªz&¨ÒZ?¦@·
pҍ?£¥beԓP?í#¤ÄN'³? Úqz´Ä?‰pU舔ø?€†d©$E?³´Ï zWÌ?å7øA"§?ìóá,e:&? ¾º±Âÿ?°‹¯Ì&Yþ?›™') ­z?ŸUB¿S<?"ÀŠÓ˜0"4FGL J0753.9+0923¿áTyîՆ@2g,®À:Õ±°ç"À<ZzyBáý@½sO­è0@¶¾`"‡?ÈïèÛ¡&?Ô¼K?™s@>¼ž_ç@h	S»¿?ïýCÂÍoŠ¿â'‰¢€õ¿âzSƒ4Ó¿åùP¹Uø¿ïÿþÐñ?í–Ö;
˜	AGNbcuTXS 0751+095?ï~ÅÍXü?‡Ì÷Ô)?€Ä¨¢
?€!€"Wºæ?*Ô5fc?{*E	ɒ?í¯ähó?±ñ6Ô5Ë?'́‹•?¢8½É¤½L?«ñÓt]k
?©ƒ'zUå*?ëf¦	?¤3LÓ#n?«dh%d‡?–«Òi%¿?¹Y–½K?œ>"†È"7?íCßU)•]?œc—W??'#gý?Ý!°.?±XD<ìÕÏ?™™§ZM#4FGL J0754.0+0451¿àáöj*R@0$ã—­À:|­""aTÀ<~Ç¡é@ÔÈÜÓ*4?ü(æÞÆÊT?Ææ¾ûÓËo?Ç­œZêo@Wþßn@RbÊÐs?ïà&±D±
¿ÑiòâáH¿Õ'-ks¡¿Ñ´Î¾¿mê¿áarŒÖ¿æêB^IasAGNbcuGB6 J0754+0452?î‹l‡Û²?œlæPw݊?pþÆ3õ &?eC=¹‹tú?¥/Àq è?›¼cJ©ä?îø¦øÒð?žtgÊÓëP?f)y˜·ÊD?xhðm?ž%ñ²‹N?›Òð8ܔ"?í˟g²@Á?",TxK?€ëéeZ?s"%Ói=N?¯AŠ'h?'e!Ù`?픞Ø5.I?Š}ZŒEb ?"}GÊÏD?khr 9D?°ØY•]3Ò?ˆ§HÛF4FGL J0754.4-1148¿ÀôÂÓ,jö@ w9°$öZÀ8À"Ú›§À;­c¤G@êìž#l@?¶~¬®I?¥â‡ÁwP'?¶×ÉU"@ÅÐãe–@	û?ˆ??ãÕ6":¿×æÎÁ¹Š¿ãR­·]Ï¿¿á¡'bD˜¶¿àkö"o³í¿ìGÊϜŠæAGNbll3FGL J0754.4-1148TXS 0752-116?ë1ÊÐJ8?µÂIõÈÛ?s¶W	ZäB?pÇà‡4s?›"ŒH†?µ9µÇ;µä?ëA1å´B?ÁFo–ÚUñ?†£^¤e…?—ïzöêÕ¡?Á'Â'8¡?À§?XšW?íK~ãa¶?ŸvN腐Q?"Q÷†Fw?"Õ%V¤?°‹ ½l?˜G-‰¬?ëÉ]†Nðœ?™1ç¥\çC?ž!Œ'×k?"Pqh,?º,°© [?—þ-×°¡4FGL J0754.7+4823?㩔¥'ʺ@>%–À8þáv§ý
À;æêð¤Bj@ào
¤É£?ÿ¸lrïá¥?§Ÿ!Ìa ?¶	8ãÌB¹@Ûwb7,½@P°ò{³¿áM¶ígw¿Ý;$-ܲ¿áQ"'›¿ßbÓ^â8š¿ç—'¾
è¿ç½w>û¾RAGNbll3FGL J0754.8+4824GB1 0751+485?ïÞlFºj?}ÑBð™œ?D[THS‡µ?M¡Öÿ.¹¸?l|ä3k²?z—t½¤?ïw"þ(vð?Ðò:9ƒñ?VÌïi?b
?d¶+ZXÞ;?E"ˆºW¬?‹Rˆ©ÒŒe?ï*ÕÆ`mº?…NgáX¡?yõDQ|.}?y\Éã?Œ!?"'ö"=?níAZ3¥?ï"pâ?o9Ô/¯Ûq?b¯''°LX?OL»Pc'?†8bÎ%D?l·it{ˆÅ4FGL J0756.3-6431?æüً]QüÀ1¼¡œZÀ:֞©£ÒØÀ< ö¼Š@ Š›QT±]@´¨+-?Çù¸¢ž?;1%ß/?»hø=¾Ò@€?Œ‡ã9?ï•[¬£7¿æe"®£¿Ìw3=D.-¿ãE=¼h|¿àgAøÈÔ¿ÓK‡½ÏAGNbll3FGL J0756.3-6433SUMSS J075625-643031?ïX	P݋&?ˆqùndåç?Ul´6œ?Mqt}ÌRO?"¥ÿ.µ?‡wÛìµ	ú?ï:x²Ì}Ó?–
ýõðž?R_Ú²O¹ƒ?bá K'?—ŠëûKJ,?•‰²÷òZp?íé·üR?·ŒÞf>»?u`'¯d?cYO±ìË?®ÌH‰ŸDì?ŽuÚªô"?íªÑׯi¬?'CÈÐlœý?vYžsBFÉ?eÂC%S?±C×[PŽ,?'Ó•ˆ°Ç\4FGL J0757.1-3729¿ÑJU÷áÖþÀß}úâ~À:­"àòôÀ< F.¸z/@"æìސ?ûV¯TÊ?Íá c6?ȄiF?ªe?ü¯©öÞï@ìIŸSÃ?âSˆ¾*´¿ïÆ~ŸBP?ïÿú÷''ý¿ÙiÉ<Ÿm™¿×c(ƒ×»h¿Û`~oòAGNbllNVSS J075714-372734?ß9ÑôbÆ9?Å©Œ}wŠ?k' 'w¤¿?a³½IK_?àG"åL%@?Å¢YÑ}9Ç?Þ`ò™êX?Æ·ê(áj¥?acyµSc}?uëÊü'G•?à¾#9U€?ƔM¾¢@?çœ×ìkx?¯™zPº‰H?ŒR¢c÷þ?vÒ$ËCƒü?Ñ1Ó	O?®"µ42«>?çôvΫ ~?°û' ÀÜB?ozàÏi?iÃ{¾ñüe?ϱæÝ3úÇ?±'Á]	4FGL J0757.1+0956¿åÅ&³#Q@3Ø{V¸À8¾Ø»™À;ëùŒHx@
Òw[¬#@ý¶ÿÛíÒ?¤™,v«®?£Ï@ ?þçp6ÉÀ©@"®%lÌ¿ÄÙn[Ra!¿ß$ÑÜFw¿ã<æÀ"Ùf¿â¥ôñ¯e¿åC5ªøh¿Öß³#®ZòAGNbll3FGL J0757.0+0956PKS 0754+100?ï|)œ9·ž?†v6ñ"Y_?Pm>\µW?Dºd¥»b¢?Žçñ%ûf'?…í¿Õ?ï0é)©ïû?˜.',c?iÓ1ÛA
?{¤O•Ü?–¨t¨æ˜'?"æìɑËÄ?ïtL,gÆ?†lšgkÑs?r]c'i€¾?j¯Jô?™ú™Ø§$?ƒC£c}ö?"n?Ž>ó¿ž?‹Ÿr×çP?ṽÿ•Q?Ÿ:Š´¦I0?†¾±à••:4FGL J0758.1+1134¿êë¸ö+@@3ú\å´$_À:ŸÒ¡"$À<}၏·™@ˆßµ\Ã¥@úz¡'¶?Àñ'êRï'?¥B#ªÃÒ?å†Å&6@#¹˜'‰?›v«Ô¿äQ›2öÍQ¿ç7"+#¿ÜWGd˜…ó¿æ¨î#;n¿âLÜõ)AGNfsrq3FGL J0758.1+1130TXS 0755+117?ï6Úm†?""±ïãè?i=© "?Z?ZWäzƒ'x?›qo~>·Q?'ŽÒԑx?ïr
~	þb?‡hI&´"?Oy´r÷?[Ãø'W?Å"uêJ?†[úéc?%ý?ŠÔ÷þKÅ?tSkU§Ò?`€@qï&d?¤ìp«»'?ˆ'Fû½9?îÑÞ^Ý?€iß^Ú£K?u
†›Fü?ZoCSÆ? @Ûi>Ǝ?§üe'ß4FGL J0758.7+3746?ì?¡3Òüx@<áµ ÝDÀ;+"7ÉÀ<³bØ<l˜@\lû+@èy=Ùc?ÏBH¤ßrí?´~<Pé'?å÷SSd+#?ýœ"Áéð¿ï,æ}wúã?ï¬{­¿ÑPÜÚ¿Ö!yÍKwο꫇½Ï¿ÅoU®2XAGNrdg3FGL J0758.7+3747NGC 2484?îü_=Ôª?™³·›9۟?hV¹ÜlFf?a$ð*¼åî?iA	òAß?˜ÍzÂÈx?ïp'êsì
?Ü¦pPAº?X^v âK×?evà{èû?gÛOtZ1?Ž½ƒpô?íGBÄüñ?˜ÉBïM)N?'Ú7Š†Þ
?"¡­²¹Ž?±Oa¿6`î?"÷!ºZ[?ïšå†ü?€Ñ,í­ï†?€0+ô?mjÓÌù?•4¶
Ä&†?z,¬÷Ѹy4FGL J0758.9+2703?ìÚépœ@9ðr° ĜÀ9òÛª¶"À<mžƒä%¯@R­²«8}@Òáüߺ?¶'›}>o?ª°CÃèçN?ñï
D& ~@yıJe¿Ýpä+Ž#¿àJ¾ëÔ¿ãÑ.[]¿Ýó‹=
w}¿å'6É?¿è7fhê¥%AGNbll3FGL J0758.9+2705SDSS J075846.99+270515.5?ïl5Š†•Ï?'£±ëϏ?f½|`¥?X@"^–Íb?lmÿB‰e? –?hhÌ?ï{Êï Y?Úãÿ4Ïf?Zê/ã¬0ô?ié[zxã"?¯þ†ãÆ?‰¹Wð·?íÙþ†\‰Ã?'ìaÅõ?…íæôöb«?uÝÔˆX?¬äÜùË#?£"GÊ<e?îø&}Xéô?€Åè£t7?‡
ŠgÞk?pG·ñ¶?•uë ó‹¸?x¡5ú8Å4FGL J0759.6+1321?âü-["¡@5dàTiÀ:l¸ÿÀ<eä«æ£8@!K€0¼á?ú™C¬Äð?Åޒ\ŽvP?»«w¯?÷)sçXiN@®¡úçr?ï'h@Žf¿î˜›Ø8:Ú?ä^C¯'9¿ÝʢԀ˿Ãn9ÙënN¿äyT¼AGNbllSDSS J075936.13+132117.8?íÕQ©ýÕ?°3ÿ/f_ö?Yõë便?_û})Ý?°í›~\?¯Ö#üž?ïg½™¬ìu?–kòôs-'?Mo4¤™Î?[".ߗì+?'Ó%=£?•üˆ(M}z?ìT±³ê‹?©8G9Q§?i'#i­?d.‡4'ˆë?¼'îO"â?¨þ$´ž¨#?î^¤8z?'6œëÉ€?Yg:
²‰?R£áCe?©J†æ
Ë?'ƒt}>4FGL J0800.3+5611¿É?'țå¤@?³df±æÀ;:V=#wÀ<ÐÍ;‡•‹@ ­%èqï?þJå†×õö?Çy €"?Áþ"ÅõB?øÛkEÉ7í@;‹Œ:¶_?ï¬)¿*å¿Ø±ÁQ™{¿çýÀTïEž?î"ó—'Ø¿å€ê«Ú便åŒXž&ÇAGNbcu1RXS J080017.3+561116?ï`Æ?G¼¾?'áóoí@?_£Ø÷ˆ°?\HÏãLÚÂ?'íÉxï§?âõj9»?ïXi`™4?SÙÊΦ?[2Íµæ –?fRA°:t?"?¡8Žw`?Šouµi?î
o´ù?'»Ábñ†?v-:Ï$$?aV\Ç&Ü?­±ªËܾ?}ô"úL?î}ù«¦õ?X õp?ë«F7?€ø_ίéw?¥¢JÛ"Ž¢?Š"I'3‹4FGL J0800.4-2257¿ç–ÿ¾ð@
戢ÑPÀÀ:L1ž½dÀ<S±Wü@@*°,Øü@…/‡­?ōi(dM?ÙÁZ]™Ž1@w¡øì@`[ÁqÏÑ?æŽMÀÓm?ÀÂQÔÒ*¿äé¾4ù‡¿åîoês¦Á¿ïÿñ7n+¿Ù¼®;è
›AGNbcuPMN J0800-2302?ßÍ7U¶ßè?ÄV—?Q±?Ñ)Châ"?ÂéÎ
… j?Î
'Î
?¼'"ËÞ+?Ýf1) É?ÏžuVØ$?¾"ÎQþ?¿œòÑÏ"?ÛI"Ë•?ÌYb²ÛOª?ào7L`ƒþ?³ì?1Y?ѧó­³j°?²
êD±?Êó;s¨?§þÀﭝß?ådëP³54?§ž	þ³œ?Ák"ÂÛt?¢.ï^†'®?ÉG(pO¿?¢ì| 4FGL J0800.9+4401?ï"צ֪,@>‰ˆÁÛCÀ:Y:ßÏÞÐÀ<ŸOœ†@'ä¦èb@\ºÞ¿q?ÀuF©Éô?ÁGwÖø@1œZ>:@
åÜæuje¿ë¾«Â0O¿À*lD̹¿â¼,5èð¿â$!È`¿åeˆ…ug¿êœÞ|w AGNbll3FGL J0800.9+4401B3 0757+441?ïñÝ ½÷?Q|˜"(??79bÖëÔ?<ß½+-"?Twð+\Cr?L"+Ií"ï?ﶏBÍB¢?€Þ‡J9›i?ChEÎO('?W£Á¦ƒs\?%ªïÊdÄ?~ÏÜxÂ\þ?ï="‰ç
?~Œ3è3ó­?m6}Ù©î?fƒÆf ?"¦®Óþ3?yÀB?ïÀ8îæ‰W?c 
¬'Á?]°t(	þQ?GYå++Þ?xwk'¸Õ??a˜Æ¡ôW4FGL J0801.1+1335?äeˆžÅ[@5yj&åGÀ;UDêÜ0À<˜'6ôˆÓ@GCeÛQ@oå]½Jy?Ï_×@™"P?®3‰ð.PË?â{wN:@M€VQ›S?êم!½j?à-‰Àނ¿ì\Þþ'¹¿¾_g¥«¡¿év±'n"ÿïÿûbâMhAGNbllNVSS J080115+133643?ïIfÏ¥{í?'lgO	?m0¢·Ï(G?cõù²£?"-´VC?'~»ohöé?ï Ú"r½?˜WܔÕ|?dB"(P6?v¶™ÑD?™Q	Lžh?–ºò˜ÁÀ?íGì"zÑ?š¥õ™¦ù\?ˆ¡'A@m-?}ßdYÌ1?²¬lÞÄÕ?—p±J>W?íyþ—×5€?™€€9õ
*?•
k,ž¢?…Výôõé¹?­ÕÌöX¹?"ôy€o}4FGL J0801.1+6444?ç¼K@¬SÂ@?¿#FV%§À:ܯæ8óÀ<ͼª R@ïÛ›l@^	Zõ?ÀQמ?Ž_^E–ÉA?Ð(€ý–nA@±ýx¼)g?Òdè'4ù¿å|, oa7¿ä& Z¾h¿Ú•ï ·E&¿á?›÷Aë]¿àLÜ¢,æAGNbllRX J0801.0+6444?ïáYL?øW?sá¾ç²}h?>r̟çå?74­`Ç?jØZ,
ªÇ?rö‡A,<Š?ïÉs\o`?{±e³ÌŽ¦?1ÛüH¢­?AÇë…7íÃ?zlh'ŏ?z"˜#Çø?ï!Àã¼Î?ÅÀ!"LH?aڅ«GÓ8?WWhþ·?™Œ'èÿkÜ?€Ñ'³áº?ïÇ^Ÿ ?c›¥ÁáÓ?Kɹœù'?6õ¶!^
 ?x×Æ|ÕF?c4S[p4FGL J0801.3+6631?Ê3XK_hµ@?¥yžQ?À:Ö§"þÀ<£dύqm@î8­Ež@©¸ËŽ?Ë{«r	1Ø?ɔçÙ³Ñ?öl×[œ@¨»R¦ëè?é'ôÛߏG¿â̎\X¿é¦Ê;"¿âa‹¶'¿é–lˆ¿Vÿïþí{˜ý'AGNbcuGB6 J0801+6639?íz
ë	?¦`ÁpYޞ?•÷¿°†u—?'ÄäÏÊV?­cN¦ž¢?£Ÿšlç½°?îøŒ<>JÒ?•A͜ž¬?hÜjAÐ?nŒm*v°?ÒôÊî…i?"«Be?í@"il?™­R°r»?—þsrʵ[?‰«?û˜?±Î^‹*K?'Åx w?2援?'¬£MÐã+?ÝðEVA?rNE¥_?ž½!˜^-?~Fê~áN'4FGL J0802.0+1006¿ÖXÈ×Rjd@491"·ºíÀ:€®@ð‹À<zÛmy€@Ÿ*Þzõ?ÿM"þ1ɧ?Á#ÖÉÐÃý?¼)m↝?üI¬|]?ûÌpk¢æI¿î1ºÂß
A?ÖW•}«&Š¿à C=¿Û|ÂHds¿ä+"Xœ‰¿âr¼Jž‰ÃAGNbll3FGL J0802.0+1005NVSS J080159+100535?ïç×Ô?ŽO²Ë#ž?nVš—†a?odƒTx"?˜ñO²$
?ŠÚ¥ÆY«-?î3³i?¤Uùäu™,?ˆ¯'¤ç"J?PRŠæŒ?¨£¸[Š?žÁòvüa"?í÷'ó%ÄÊ?çÌnÃÅR?€€‡ãÅÛ5?pùE	2›4?¬m^Ô²<"?~…×±VÙ?êÖϞ×1?—â:Üï´?§JÔÀ[|V?‰ÌÄ"uÎA?½¤©¹	?"Í"Á(ý½4FGL J0802.3-0942¿êi\\n¸@%çÄÁe~À9Ï6¿yÀ<#Ÿ¢È…@ 0ÊڄEt?ýî%\°Úÿ?¸ƒ|-""?¦Öñ`Lh[?ñ7¼šO¡ÿ@œ•.ûÁ¿ÕTúe
¿è‹Ëz½5€¿ÞßeUÅ¿Ù8I½¹3"¿ØϹü‰Ð¿æŠQýù•ƒAGNbcu3FGL J0802.3-0941WISEA J080215.63-094250.9?î@üvþá?¢×V'¦¾?a©.ðPž?TÝÎvÄ£ô?ªÕ¨œQð?¢†z`L™-?îs/=,·?­'!zéØB?Ov¦U=hä?[KÁOf/?¨O42Ø>Þ?­x9ÒZm)?ìü7"Ô™]?Ÿ}•£
p¦?U3"Ϫ±?rE¯®?µóœðÁ?·?Jfjîj?íuRÕöyè?' ç†?tÑ4†ù…'?`Ðá¼à4?³Vܘm?±Mšíț4FGL J0803.0+2439¿çŽ'iä!@:»'ˆÛÀ;o"1zÌÀ<ºëªÞe|@ á:á}]ú@¢(ÁÀ)P?ÂX\›D¿¶YXê?ð·…Ýúòz@ýµ\Í¿":B¤â1¿âùóv"Á›¿äï:€.Ž‰¿í
DVq%Ý?܌%þpÛ¿Á
ôeB$AGNbllNVSS J080307+243749?îmúI®ü±?ªI
3‰ô?nt£_'ã?t%»˜{?§9/§?© Ÿ'?î%×íªH_?¸Äkêó?w\ۚ`»?"œ3F˜t?ª¶ýIè.?¶£®B(
ø?흜•°vS?"›ZOûÂ?{vsE+"?rö'¯qÆÏ?±[ºÛGú¶?'Ï–~^÷ ?îL ğ›?šÿ*CÛ?H$2ËF?Mçùp]?ªÕnÿ=;?šó#ÒÙ¿4FGL J0803.2-0337?r_!K@,b€àe0À9<IðuÀ<3{W3@=ÚÞ]mï?ÿ×¾³.–?ªu¾É?—Hº²™?æ—VO—î@	íÄoÜû¿³ÂA-œÆJ¿Ý!4ƒqý¿áwÂ^´Á=¿ÞæNþë­ã¿æÑE7Aµ­?•lÖÂïÔ9AGNfsrq3FGL J0803.3-0339TXS 0800-034?ï‰Ս?'-†,éî?G%ÂܦA"?HÝ/~ƒ9?ŒF ÍÀ8e?'Œêœª×?ï¡À©h?Œ(bJþøë?I:¥êˆÞ»?`9#ºÑŠ?…ü+GR+N?Š',®ëÕ(?îí¿Ï!æW?…«;'CH?qB;Jêë?h˜¼˜á?÷wI²?ƒvĆô‡?ï>òŸ"?~ÒÂkºá?pQ¼rs—L?[VtÉL7p?"*€'§?z{^M4$†4FGL J0803.5+2046?ïZV9adc@8ÉDg8~À;9Òïü|¾À<¬@ä@)°-ï#?ÿüS"¾?×7¤¨§ÿ?襢¡€è@	/ËOKE@
³Ë'åö??ïüÕ,ß¿­%ëbd#¿ä'§C¦Gþ¿ïÝu@ô¼Ö¿ïýè-{cN?ïpÿь$AGNbcuGB6 B0800+2046?ïŬbظÆ?…ªÏN´³?HbYŠØQ?R;­…x-?zƒbaÂ?"†uLœ´"?ìíëۘú?·Æ2YU? <l5ÁÛ?­UÓê¬0¤?°"RkWC?«(fý?êÛÂTû–F?¤Y™{b!?©ÿÈ«!,?"©Gã&*'?¼"	'··?ŸhUËùê'?î59›"P?—
½—l?ŒÂŒÁÒ7‹?'hk鬹?¥{̵Ò=?"¢›Ï/4FGL J0804.0-3629¿ÁC·dÛ¡ÒÀ á÷×<'À9ZÙæÃ1À;±¦Ùóü¼@ ¨%o{8?ú±À×ÌP?¹+³b¢3?Í/ö¨=vX@Ýð
¿w@{)(î5Ó¿èÁÿ)%¿Õ¶º¼©éô¿×¯[bQXã¿Ã(™|=h@¿áéñ€‹U´¿â	,«AGNbll3FGL J0804.0-3629NVSS J080405-362919?î¦f2è&?"÷òt?'ÛO¾˜¢?{ÿ_=_1Â? âÈá×m¶?˜­%î_¶È?ä)ìïÁŽ?Ë(üXk?hwÌiÏʗ?xA¯F?×{85LÝN?ËI×që?ê=™?Ý?¬±
móC‹?³ø!=w?¤ZœÝ—b"?»7Tûä?Ÿ&´â½¢ç?è6D.3%n?§' óæX?•›t°òê?}RIs¾?Í;؝Kë?§>ŸÙ=b†4FGL J0804.5+0414¿æV>&ÆE@2.úÆ\À:a(	4À<U°i@íÊt­Ñà@œn`/ë€?¼q{BkŠh?¸LmbÁ?øNI¿f²½@
bK¤™'?ïýêa2Iÿ¿ãŒnØû¯8¿çÎÛ/f¿æú¤¬S¿èX<8d¿ïÿÈl뻥AGNbcu3FGL J0804.4+0418TXS 0802+043?ï˦ˆVa?š^ž1ùË?bR=¹ò›u?…Àt2'?qœ÷ý¯?˜8ðYÃcT?ïL¶]ø?–¨ëJÍ?_8Öüår™?rE‰Ú]×z?"Œ;ÍEéÏ?" ûû"l?ïP¼7>)?~uQÊ&Ô?rEš13ë?g§-Š-)­?˜‹î?{{$i')?îÌm\<—?vkq"À?‡–7rUŸ?l÷ým ½?šè˜¿B?|PÚô<Ù4FGL J0804.9-0624?Ú÷›3û]@*Xä2DëÀ:‡ö'À<'õ»Ÿí@ ˜¢=W#}?üSd"?À©õ‡V ?½=ú·k¼'?þ;ýÝ@³6É?Ïy?Ð*ý$"®¿À
~ß06¿Æ"àå]'W¿Ü>&áì¿Ûm·_þ¿á¶óF´xAGNbcu3FGL J0805.0-06221RXS J080458.3-062432?쯐OTݏ?­&¬Ò?Yý?FÉ'næ?|^¨ˆÐ¼?¸éƒ€?¬pӍ¨ê?î"®f'è?¨DÒT?nœ{&'¦K?vÆØqO'?¬Lýg.·/?§3نO5?ìð#.©u?¢~€ZV?J?Žü~¬9`®?~4'U–2J?»Hïˆ?? ~øÃ?ë? "Äÿ¢?'5b–ã‹a?'_ôMßü?uIÉì†6?À×#IÅz?'эsLQ4FGL J0805.0+6746¿î¢«Lä#@?䖚
Ø¡À;'çv¯ŠÀ=Ò®Že@¹+x~ÁÒ?ý3o~=Á?ÔJÙã5ÄÞ?ÜדdÌ2s@dZ˜Ó@ºŠ.¾³¿ïÿ–þߙƒ?ïÿ·pD5º¿À@˜ ¯¿ä<UxØY¿ã¬(|öˤ¿ïÿõƒ¥;ŽAGNbcuGB6 J0805+6745?ïƁӒ-Ã?s˶+éÎ?d!«»«?^°Ð|˜‹?r®@Yc'?oå×[˜4?îå'~=?šñí­c©®?rÒ°õÓô?{Ξð(?ž™
úé?–"‡OKê³?ìõý±€?›"­m¤?™K"j	TY?Šë…Øçǵ?±ý.çñ¦l?•&v5ǐŽ?î8›—m?4Lîj2©?‹ ÿSC³?xêjd?'"?¥–v'9H%?Ž?}—t÷W4FGL J0805.1+7744¿ÍUžmýß@>Z<d4\ÿÀ:ƒ4-.6tÀ<{Wɼ@öFBÚp@]­Z@¾6?¹8¡ èÝ¿³éKó?÷5Ë(‡Þ†@Τ¬È"¿Ð"Ï£@âH¿âFó¤§ê•¿éçåWMÒ¿â©i»…|¬¿ê¦>"z~K¿ïõ¬EmÈAGNbcu3FGL J0807.1+7744WN B0759.6+7754?ïàÉýÌ,?iC֔h®j?cTkWs?bŽˆ`Ñ8?WÂç(Vú¯?ZZ.§`¡X?ïµÞ)þ?''>U¡å"?BÚ­=£V?X†ÑCFH?'' ¡¦N?€Þùᆄ'?ï*­ôˆÑG?' ù
­0?oï†ce
¶?gç5ïkh?–¬P¢y5ò?€ŠR¤g°?ïÄåƒ1`=?druñ¾Àe?`ff\Yã?O	©ÿqg?uZ9"ïÆ?aà¿ôä†s4FGL J0805.2-0110¿í†'ºý8ó@/"(ÂzÀ9±Ç²±˜"À<,<{±QF@W¨—ä7Í@ÉË«d9?´"D•ÜÑ?Á½…\ @çüMÃØ@ ççÛF?vRdë€Û̿ݲ´Þ¤'¿ç¡&Ö-Ÿ¿æ
ݹ.4¿êö&B4¿ïÿÿ>¹úAGNfsrq3FGL J0805.2-0112PKS B0802-010?ïÉ°MêÚ?ŠÎâ>nH?WMskr@û?hGõEÔ¤¡?uT|].œ?…!ôC¿¥?ï¯AxDJ"?ƒSÖp‰ù1?CIeÉ&ƒ?X\5Dræ?'û'Zù|?'3îÞ­Ö?î§å|?‹QiÍ9?…Œ›"ë[?vžÑ9ø?žè=N:·?… ×¿ÝB1?ﴜ¡P_ü?eö*î>¨0?\@¢jR%?FPÉK^£?~®ß/5m]?cYO±uÔ04FGL J0805.4+6147¿àƒŽâ¨Ï@@.}ªOÊCÀ9ºi¨:FMÀ<e(wŽ'@k`ÊÆi@$>úè?µ¶e)O…?Ǟ^ºËm|@
k4*©ø@˜‡C'&¿ÏBi‡¿å¤ÇÛØX¿ë	øÂ!¿é»©Y*=Á¿î_Jé2^!¿ïY/±žsAGNfsrq3FGL J0805.4+6144TXS 0800+618?ï³XŦh£?yòIŒNGÅ?w¡Ø¡'"£?q)¸~µƒ?mc‰r5H?lw|<=$?ï—PJšç?ˆÎ»$Ï	ÿ?N¬æ·?á?bN¯,ø~`?ˆAô¥NF?†BþÃlHS?î>õ	^Á?–FQô»L?'°¯uvç?†§;[üf†?¢¸W¯X ­?ŽQ«HÆH?ïêBveOã?QM½É¢™ù?P¹'—Ïw?A[Ê<Õè?ZÁ' ©?H# ­BgL4FGL J0805.4+7534?é:é»èE@>Ëeºnü7À8áhSÀ;ÿ.Y°@Aé~3b?ý&ÈVE†ó?¡'ccý?™_»…iÐ?øéq-iŖ@Lœ«œÑ\¿×öÞN«¿ÕHåL"C¿ßÃcl‹ï¿ÙÏ¾ï"x¿ÛtúÓÆ;¿Þ¬Âû<ÍAGNbll3FGL J0805.4+7534RX J0805.4+7534?ïä¦:fԇ?`Î{7ŽÂ?3tTÁÔô'?&èwj‡a
?hë;ðق?`2	ú?ïˆRÒ"r@?‰¾$ØÊ9¨?R(xv?bà½ÂF©Š?‹¦HÕ  ¯?‡‰7杫T?ï D¼sy?"òǐöp?h_£ñ½Îà?`Ô³Í]ì?˜ësóY"§?ƒMG­Ò€?ïq6@d"?v+OÍë'A?ml¦ø++o?YoE€Ó	t?ŒWF(Ð0?sRö—ñþ4FGL J0805.8-2331¿í¦vUæ@õĊÞìÀ:ÈlÁÊ:À<GÛZ.I¿@hÝao†¡@*':ƒŽ?Ç刚î®I?²Ë.'?îꀥ+ô?ÿÑɶÂÊ¿ïÏ@À£\?ïùåi{Ĝ¿ä(íßìå¿ãûØSÍ¿à-d‡im¿é¾@_‰ÓAGNbcuNVSS J080604-233333?æŠè™òøÐ?¿'>ßq?qF§£©Ö?c®¼:÷'?Ò¥-‹jR?¿Vw	e?áJ¼«W?Æþ,ÈÙ?'
S@EB£?Ž'§€£?ÜNÿ짝<?Ǝ++¨Ð?èĜ¡­Õf?¥Ï'äšè?'¦»
¹?x''ñ¿$€?ʘ¶¥E?¤sw)çx?ë×ÍùÖ?+=#+
Î?'Èj±øà?'?ýW,?ÁB"P'Ù‹?›ÜèeŒ£4FGL J0805.9+3834?ï÷[ùri¡@>o|¯Ý©À:¸""œÚ—À<ª#}@ëÇ8ä"@ïáÝÖ
?À5a¶©Iæ?˜â¬/t7?ÛIÝC½o@Ð2ÕÀ;o?Òïaz¿±>Y,3s¿æüz9'Í¿×ÙÜÀ4ãâ¿ßÌ´ðã¿ë—p"½'ÆAGNbllNVSS J080551+383538?ïÔ;…VWÇ?hàj…Ù?HVvÂv"?=_ê¹V†-?r×n|'®u?gSõ3?ᅥGa?7?ÖV2(?852F·m?IÉëøgC?~¹d›ú¤`?}ªwC²uÎ?îñH6ë?ƒ·'•…2?kŠ¼'ò›Þ?ZRr™ûõ?ž^tĚÏ-?'UG㯞u?ï£Èa´?h'Fï?d©_Z~t±?OՂŒñÝ?'v!‡ö?f]ՓÁÿ4FGL J0806.1-0458?ïþÞ
M+¾@,J•BCÀ;NŒ"¸'¬À<'"ØAu@mö¶@?ùéôÆ)?Ý
¦a©]?ì]d[Ø@§R°Å/@DG?"¥A?Í$‡^X¥Þ¿ïþßÙïÊÿ?ïÚ%`ÙR¿äŠÿ?:Ó¿â &`¼Ù:¿ðAGNbcuCRATES J080608.79-045411.4?ꘕ%º˜?È
̘,ë?c™Á1?•D~ÑQ\·?çq×æ‡?ÇB F0¬?êÂ]'Ñ"?ÂU:QÉqJ?›ˆXóë|?§oÀ',eÖ?Á†w‡V<;?Àe\-3iˆ?ê›RÓÔY³?¥˜o0´e?¡ØÞcäĚ?ë­:÷õ?Á}µh?£bÃg¼C!?éÌ.°°ŸC?°ØO?Šñ[8Óz?‡ø	8äþT?Ç -'‰õ¿?°ÆôO#±[4FGL J0806.5+4503?×-‡ùšFy@?«À~à°¯À:µ *­R´À<ŽIöÄ@&üª‹@ð×°´h?ÉÂõ³uã²?ÀT…h_9÷?óNcaÏ(@úŽ±´Ÿ?ïþrâÅB¿é]÷vĂ¿áJ
À2	½¿ìQµ(kY¿ïÿݛQ)¾?ïÑB*òÈAGNfsrqB3 0803+452?ïÒd§Ž¬j?wK©af}?@zånÞ(?@·ø&}ô?t¾OŠÎ+?v¦ç8\?ïRGs6g?–I*ý|?`1pE¥?r­3m#k ?"°ã–ªk`?"'ÏÖ+'"?î2©PÅ&Q?'.Ɇƒ´Z?ƒmLû{ó4?~ß/PHÆ(?§ú´Îž
?ŒÙ.‰[{|?ï¶' vÔ?lóÉ2MZ
?YNߍ˜–?MJ5bbÖÿ?~˜¸^Ž\?iê~{,4FGL J0806.5+5930?êqûó€ë£@@Ig#$È6À:}Æp'9SÀ<«Ù§¦¢—@ ¼²MoŸ@%¥á¦x¥?·gŸïôð¿'¤üñz#?Ú}"ÛF-@£I€C‡?á¶Ì7«h¿ç}€H9Ö¿ã "IÖä¿à%°"±"¿Ç-\"H¿ègõ¢ƒøóAGNbll3FGL J0806.6+5933SBS 0802+596?ﲏŠA´?—
Z;N=Î?WKÎÚ&L?MsuÀ8k?€r¿Â.
ä?–óØ9|©¾?ï½_â£5i?€zýí—S?7œr6ð †?JŸj¶
§?ÖGŠöAk?WŸ67ã?îä^ëŒR"?ˆáÔÙú?d'ñO~N'?S*Ôsÿ? qâ2BòÙ?‡Ý"܋&à?ï"ËYNp5?qÈß.Q,?Z«ó2]â>?N'€éÁå?‡·«F6?qÐ$D¾è84FGL J0806.9-2151¿ã·jaÀá@fð¸»À:ÞØh'À<m¹ô'ô<@dM¢JBC@V§ý	«z?Ê0mƂý?Áw$ºŸR?÷;º‹¨â?ø<N¿ÓÀ?ïì²²$«¿épà'ÒU¿äX§–²^Œ¿Ì\!©s~¿ë~o§WÈ>¿ÑAqºWCAGNbcuTXS 0804-217?ܪg%ƒž?ÂõvLC!5?†1b@¾?'S™OаŒ?áRO¨Äõ®?Âý ©>§?×9÷6àæ?ĵž<£R[?šÊ©m{1ï?ž –/ä0?㌯$þ?Ä^š-1?èúóþ˜èÏ?¥©0S˜â?"àGÔ?uÅcÃÃC?ɀtSbE?£Ù¶`"¥_?äð2"@/?©‹?#EwÌ?®€KjY.?•¾PõÂô?ÒO'N4¯â?¨VÐ#Ð4FGL J0807.0-6102¿ÑKØØÁ2À.¾ó'ªÀ;¤˜ÑÀ<ª^Ô¡­d@¦/ÕÔ¦?ÿÜÀ_×?Σ:Xš¡?×êÈ@ +š@F™&­ó@ŽªÙÝ×a¿ïÿý`éNä?ïÿþó…õ¿Þt—A$¸q¿Ö×=¾ýVW¿ëbÛ, Å¿ïÿöùŠpAGNbcuPMN J0806-6101?ïmøÓ2ù?BQÕ¦—?"]+}Ö ?'´Î0Ù?€-dŸµkE?ƒw-pë?íïÁº@?®dz¸ "+?Š…š­'Ì:?'ön¶â5?ªm]9ì?©"O(¢"•?êA ÜI?¥îÉk¼Ä?°ø*¥¾})?™Ô›'üÎ?¾•ÌYZ Ž?ŸÛo'†?ë?ë'Ñ£8Ùg?œ,ðf?p?¨
'ùägÜ?¨¦ú+PÉ?·ä)iGÚ?"ô×3J³4FGL J0807.1-0541?æö­qùÓ§@,VߋÀ9Š]ÜTÀ;³›ý÷è@v©÷	â,@ÌúÕS"?«ã!€‹ß$?¹"€z䢬@
 sÃF;N@
¶áQê?î¦xÚÝ0È¿ÖE—¤Kú)¿äp5݇…¿àaßyw»¿åþw4ÿì6ã¡¥¯AGNbll3FGL J0807.1-0541PKS 0804-05?ïºùôD®?Ž*¾È«%?:ìÏ~9é?9¼ÀcÜv?€¦ÛýÀ?Ž2NõŠ}?ï˜_¤
è?Šeº÷_?Nð`:¡¾?`5rI"ò?‡ùõS5:?‰´è›n"?î¸ÌüÎ Ø?ŒXðj^E8?,ºÇuv?v =Ú? ˜Ú/C§?‡<ccÉ?ïDÜ'à}ð?z®‹H\"?i™o'Á?TÂ/p‰ø?"1IV
¯Þ?xôñšË¿14FGL J0807.2-7630?ïºKLHqÎÀ69†3‹HÀ:‰: >BÀ<pâkš'Î@ÁnØå@î€F}?ÃTAöš{—?µªZ±ý>?ò0œë]±Œ@	ÁŠŒ5'ï?°	/(·";?ï lf±¿â-颛uè¿áª}?Æ¿¿ãt¶‹Aè¿éiõ1oä"AGNbcuPMN J0807-7629?ïç)hʨ=?"W(†Z›Ñ?9åíþvp?G@ÚhÆ_?e™Ùu—"Q?ƒƒ‰0ad?ïÂH‹Jn€?€ä—Wgië?1˜,û¥'?Eë+íVä?}Â:Gùp?€JFŽª.?ï;h7?'P™¼Ër?eŒo˜ÍÊb?VzF"÷h?™§¶|?|¯<kÚ¼Ú?a"TS?oš¸Å?h¯[P'þŽ?W€®J*F?‰2ÆÆkü?lÀ/#aY4FGL J0807.3-1954?éÃëUN@Ôó…À;e*ýÌÀ<r»H@
²@ØhOõ‹³@V—:*?Ë"-;øS¹?±åޖ£Åí?ëV—¼IÇÊ@Ò¡ÍðŽ?ïï"Ê/d¿ä6A¥¼½‹¿å²>àæ¿ä"8säÔ+¿ÔUÞXæK¿ã!ÂUO"AGNbcuNVSS J080722-195218?âñðÊ[?Ãän??pëe@7*E?cÑÂÊ'®Ç?ÙÚ.‰k¢?Ã۞L¤ì?à²Ç‰UT¡?ÆǹŽc½?{ƒÀ¬™5‡?ˆÞ"çª?Þ,aê¢ñé?Æoåšç'?èêÔ÷c?¥ºü§S\Á?Ž~!Ùýئ?tÕêÂÆív?ÊožŽƒØë?¤˜úÇ~-R?í'hIN?'âР«^'?qR{™‰N?bÜ[§¾DT?²_•ûöò™?'y‰´6—4FGL J0807.7-1206?ï!	±ÉU
@%ÂÂ7G"êÀ:~[ãU¥À<;yQ$µÂ@~!IÑ°6@K>WS£ì?ÃæÆÞvB|?ŽZYñ@¨?ÆѾ¿@	è,B©ï¿â®˜™¿YG¿ç²Á-Ý3¿ç[bA=·ñ¿é8'â3n¿åõæ×:¿ïÈc`øh\AGNbcuCRATES J080736.06-120745.9?ïßf½s;?n2"©(Ò?3U7&ʕ?+':-¬Ê×?n†øû§ë?m¦'5c(·?ïe§('áa?¤R1éN€?Bñ€ûH.?g5µèÊ3U?'³Žåɒb?£³öxË,C?î`ID­Á(?ßa²œ{ü?x~*k\.?m'Vd¸æ?¦ë¦g¸g­?³'‰Åmö?゚Áyv(?dùô2±?GoˆƒíYô?5]²\¾$Ù?}Â.2Ç@‹?d`m	sH.4FGL J0808.2-0751¿î¥WIë@*R¾H¥‹?À7‰²gƸ·À;Vd'PÐ@¸éö©?)@å*"8…?•e‰Ç"~¨?µR3S"|¤@ jvSCsó@¸[äWX¿Ä®YڑÜa¿ßÃt
6¿ãk–¼o‡w¿ãž4"䤿æï9©nù³¿íRuÚAGNfsrq3FGL J0808.2-0751PKS 0805-07?ï–~#Mí?Åõš²ê?FõEv@«‹?BG¦Öó?ˆñ"Õ ³í?C?7µg?ï>4†xÖ?¢E9ÉÀ?ež«boÅ;?€õËmÊù?•…™Ä¯ìÄ? javØÕ?ïóì.£?Ž|<»íÎô?‡ŸA

¥×?…"?lÈÐ?'Ñáõ9ØÖ?ƒÒ{þzÁ?ïÚ*mi?dèÔ£'s?=ŸÜékÙÛ?6s|áB²4?qË|å»?cãôžtIš4FGL J0808.5+4950?ì}&/Oßø@@EA [ÀÀ:
é¿KÚÊÀ<n«ï³x@^'€L–‡@¨1­!5Û?¼µ#7èz?¾Ô»-½þS?ù‰žsóî@©A,p ?á?ž{«¿æ¶<½u–Û¿éfæÀ¿ïL´ÔQP¿ïüð¡=Qð?ïûûùáAGNfsrq3FGL J0807.9+4946OJ 508?ïå›ø?ßå?m":"?a«6€À¢Ó?i½Ù¾®,?Qq¢~¾ï»?SCc`±?íÑlø¥TÎ?³_5B†?'þø{e?¢/n
ä­?©é´8%?©G»r¹
?«Ä?Œ¨)~?Àæ?€Oõ·o?uþœÙÛ-%?£Â÷Û\È	?ˆ²¦'\?ï")ü ¹…?‰ï¹Öy­û?'¸>ÒT&Î?…ôLn¤·à?"3)Pä?qÿÙ8¤g4FGL J0809.3+4053¿êº˜6)@?""åÕ²OÀ:Zi¡"I¦À<yèÿ2z§@ög¢{•x@ü6ڇ s?Á¨wB¯Ã?ºzÈH-Á.?÷ oz@
6H°HÕ?ìø´¢¨ñ¿æ6¿áa¿èׄKS»i¿ásï@j(h¿ïÿð°×£À¿êëÒ¶ñ™5AGNfsrq3FGL J0809.5+4045S4 0805+41?ïà®]C?eéªVŽsì?Suƒh²¾?PO¦}¼ÊU?e–áá¨?`Èêþ'?ï…8\wG?Š_Îcù*Œ?RëgÁ8—ù?c*sËP /?ŒT{ê&â?‡ç¨Ð(?ï]c†Õ«?Œ·»"?sAì l9ø?c¾ÙFEé?˜ƒØg
<?2cðÑz?ïtEW_?â?rU·´Ì°?xmÃOÆËb?b²£AKN?†·È€L¡{?k¶,áU4FGL J0809.5+5341?ÔQõf‰@@vQ ÄeÀ9OM½øôsÀ<w^o@ÿ½ð÷4@QâZӋ?®2ó'Þ?¼ç—~aYâ@¶î·`-@
+m—C¿á+}âƒî7¿Öļþ"°.¿ä­'Lž>¿â±4Ur"\¿è"âÀ*'¿ïÿûbâMhAGNfsrq3FGL J0809.5+534287GB 080551.6+535010?ïâî
N³?fùÂ:?KPƒC9
1?P3ú´ÒG?f=ԑã
?aÒ|0nf?ï±0û·m@?'ې"Ä?BYµÉÍö?T3	ôa?'"{vÈ=?ûígoà"?îÒB$ÿÐ?¾}ǖR¢?"Ô*–]36?€þŒÝ?°Ï?›M¦×d=?‡/¼ñ?ïïh'‰š?K[P>æ?1C[ø"Z5?!»pËGù(?\ÞïÎ7Ò?IrŸÛfö)4FGL J0809.6+3455¿ÛhC"Ü@>[=ÀTïFÀ:—öÀ¼RÀ<…¬bäÒ@ ìKœ%?ü­,SE!r?¹½0EÃ?xHÝ%Ï6?±o¤'½@çèF¥Ö¿?ï…[ôó]?Òà™ËW'¿ÝC­iZ6­¿Ô
ÿx›¿åOoù?·î÷€:ß
AGNbll3FGL J0809.6+3456B2 0806+35?諸˜šdW?z"/¯7:?J¯"ÖJ•W?@QÖé¡!?ƒ¦g¬@ë?yZ‰r¥è?ï™ÔWËŸ?†">{ÿ?FO
´)í?V
IIQm=?ˆ%øìa•û?"½w½Ëûö?>?‰¿K1ʜÍ?p	x•ypd?Zóç‰ê¦"?¥=Pî?ˆ|âÀ¸æ¼?=~u?…mâ@›‰§?~Bƒò|%?fŎ®é?£g…íå	G?"¼d•S	4FGL J0809.8+5218¿îó7æÝUl@@uÂôÀ7ßF€"À;WFG.@ѹ©™è?üúÜà@G?™úAú÷,? ¯·=C'a@Æy{ìài@/®'MoÊ¿ÈKÇ©¢PL¿Û ÿ-C¿ÝùVÆ'!¿Ø`Z³ª¼Ø¿à҈˜ÀUÆ¿ØÿŠÄê€<AGNBLL3FGL J0809.8+52181ES 0806+524?ï瞀?aB¦áùè?¥Ðë<¶?ƒÕ]ØÀ
?g÷Wºø‹m?a
~ÕrJá?ï¤iìü?•?ƒ÷óû"y?B¿Þ3ê#!?Q\¿u%?…¹†Ý±x"?ƒõ£Ô-Š?îö|Q‡¡ã?WûMìY?p¡>ªI?hߙ™Aä?0a1/?‹nñ×Ucò?ïáëFÅz¹?_ùã-i·†?"
fá
-/?¯;Ó2-?lóâÌttw?_±
úàÞ4FGL J0810.9-4926?妜bKÐÀ!8÷‡‹zÀ:·SŽÕÀ;ó¥è\uL@'ªk¤@K€œr'î?Ìw›Žy?¯ðRAâ?äSõ`æè?ყòͽc¿çµfI
5
¿ã݄ªõ°¿é…Áàà€¿Ý8Îø ¿åÇM1:Ç¿ïØ¢žP³AGNbcuPKS 0809-492?äËÂÈîÍ?Ƈ?õ´I?'k潫Øò?yAb8?×I	D€Ã?ÆQŽq]Ѫ?ÕK—^½åÇ?Ì °žÎ´?jdzüá?—²+ã7›?ä䊾µ˜?ÌO⍫¦'?å_TÊz…?¯€PUY^?ŸAÚlHä!?ƒZ"e	?ÓLǯ¦|³?­'1ÛŒÏ?Ù'J¿ìw?´jh7dyp?°dÒ	²H?žþæ†ò?á_×¥ÈÃû?µ=ÀgÖ4FGL J0811.0-7529?çoÿ×¼À5r=_ÜßjÀ8~é°2bSÀ;ŽÅ=jÅ@ÎȦ!'L?üûõ)hÄ?£pî!'ºQ?³@ÒÙb@{Sþ"Õ½@	.¡Kϖ?ï`ø0'æ¿ÔžÜÏyOw¿Þ_
agy¿Ûé¯Çˆp¿áD…Àô§\¿àW}à€ˆÑAGNbll3FGL J0811.2-7529PMN J0810-7530?ïj®L`ó¥?ˆwäÇP?bXÒk¸:?[y%[Lž2?_&jˆZ?†¸€n1Éê?îoˆRºh{?§þL´VAé?…ÿx'v;?š®Lj…ïN?£‡œ³»é'?¡j ÖËž?ìmHÕ(Ã-?¦ÔÒ?,"É?™‡˜þƒ?'d¡jG:?¶3Ó	b4?¢"7$Bâ?ê§v¯éÎÑ?¢ƒ'9fñ:?þ]²^
€?"Ák(ü?Á¢YŠ
?¡ò!rX®X4FGL J0811.4+0146?æL
ô6ƒ@2ìAÝ"À8ð&n(ÓÀ;nÇtž8@G4 ñ|¯@üÉð?˜ÿjÙ½¡?±ž
áXä·@]û¹I@³¥ÂqÕ¿ºž'úb¿ÝxÞ8/¿á¦.ÓR"¿à· ÈÍcÌ¿æHùµ¼æ¿âD`ý›Ì¥AGNbll3FGL J0811.3+0146OJ 014?ïÒn'T#?h3‹»K͕?@vaxG'ÿ?4á c§à?t¹êÇÌül?gØö±4W¥?ï™å§\7?‰ËÜdå2?Q^8ñ¢?aùk&Ýnœ?‡ZÒò
ÀV?‡Í/ŸnS?ïRí?'›?ƒ0USûâ?u
qT",ß?s%+i:D?_"ö€?~àºv0?ïÙýŽˆÂ´?a`üN8 Ú?;Ê.–¬¥à?."¾*Tj?qD•Ò3ہ?`¤5‰¾B4FGL J0811.9+7847¿ï顦¥¾
@>t‰ãC0×À;Z¨®àR¼À<£¿Ü#å@úËܑ¼?÷Ud;ü?á"r&Ž	?æJ 'l"@Ž{Xeó@gî¸/ý?ídIáJˆ9¿ëÇ€\±²¿Áã˜ËéM¿æ¤á@¢1™¿ïü#åGî¿Óè5=ÏnhAGNbcuNVSS J081307+784308?íÕӟYµ?ªÒ'ªî0Y?'e©)XR?OôӜŻ?©üžEu¸w?§ÔÚÁ e?íCNÒþ'?³oÒNäsÓ?''Ï"ZÆw? Åpו ƒ?±DՆôş?ª{ÔԉB?éØ`Á8–?¥PZь^ö?°šÓÈá?–£Éó#Ð?ÀQØø­? r¿ºäce?铓<€vŸ?±ç"3ôåM?«²Wž?;?)°"k?È´U{A3‹?±¸m¿'"4FGL J0812.0+0237?ïçk²ç¯@3ÚãæÄÆÀ9ðËЮÚÀ</°r#3@ Îý~›f?þÝΗ¨'Ò?¶Éš'ª·¿™UpŸÐ?s?㝺|h0?õ ôg˿1f™'?î
üwµCC¿âÆAp㘿Ù*»*
Ä¿àcJB~Q¿Éy—›'˜AGNbll3FGL J0812.0+0237PMN J0811+0237?ïÑweA–˜?pSC™vÔ?PÌKŒF¡m?Sÿ«ûk·?s:|# ?jk/ga–?î{åO-	?©TŒ'ÅhÃ?ƒxdD(²?šÒ@ܐVê?£c'ü+d ?¢O]6?í%Çh/Ì'?˜ZcQU;?ŽŠö­?'jPµ‡h?³ó}Ÿð?•_‡2ÔT?êœ7Âl3Y?¢›+³s ‹?®@èG¬?˜¬œ÷?»þ;á*A^?œ1ÏÄ,Bí4FGL J0812.3+1143¿æ^¶!m@©@76OD
ñÌÀ;«°óRsÀ<‹Q$µÁî@ͳLóùŒ@ÞÖ4T›c?ÎAƞàUk?ëqÈÅ+C?ñlÐÈÚÏÅ@±´›Ó†?Öñe]|ÝÌ¿ÔÿcÍÚ¿¿çût_ÎFÊ¿ä#@v蕿ïÿÉ
ûkF¿ïÿ–þߙƒAGNbllGB6 J0812+1141?{î™?žL"v'?s[³Abz?k¹*@p>;?'&‡±£¨g?xÞ4þ´;?î·l™ÒÐð?œœ'èd÷?qûžX6Rê?|úÌœ&Z?¢I—Ì&©?˜C¹:»â?íQûÅQa??•"œí$,/?'kíª(Îë?Î@RYø^?°Õ&jêÂH?½ýLh"X?îvV•žý?‰ƒt¸ƒ?6‡%b|ø?u³ôù‰­(?§:øÍMpé?…Êc¯Ö}*4FGL J0812.5+0711¿à
½S©d@5LP&‰ÅÀ:Ë7š¡–À<qe/.Á´@wP3:@
¸A$?½µ˜'ԅ¿‹R"Sba?ÅÀ›{œª@ˆQë…¸?ÛÏa×`z¿ë¢ÎLT¿æD‹ë[-M¿àâ4½÷ÇÍ¿åŽ)Þöšü¿ïÿ¾úAGNbcuMG1 J081238+0712?ïÔ3}Müy?oG( ÂÕ¥?U'Zƒ¯½?Q&M*¬Ð?pªÒ`Ø@?k _³mD´?ï¡HãïŠE?…§019+d?D‰-'–$?[›ˆr4?†e42´EH?"¹'@ã‡?îüÐÊÇA?…ô`9ý:?kº%lpDð?bòõîR¢6?œî¡ùÏ`?"é«þÞCä?ï›üð¶œú?mÎ,Ä?ÿ?W—iP¨?E_³É³&1?†
Ö¨C½±?la^Pp§4FGL J0812.6+2821?æ,IqZ'¥@=9Ñ쒛À:ö ‹Â[À<¨7Üæ @ƒ	ðï–Ñ@&÷ãÑÌ?¾r`ßW®¿¨õF'_/)?îA|7@èÈ€ÿ?ïåÔ`Û?ï½ö¥ä*·¿é˜+ˆ¿ãz?–îÄn¿ÊÓ_ãëL¿ÔÏÞЏ²AGNbcuRX J0812.5+2820?ïÅÈd¼ûh?uמ1ûP~?Uûg–ãw?R¿T6ÙÞ?wœóà'Ì?sn4ü6]â?ï½y%9eÉ?~ו"Õo?:¾÷Ò&•?P cӗM6?—…CÏøG?}
¦–|ó?îÁáñmÖ??‰i¥F?lø (Œ#?b]NYœP"?¢_' J?‡ðE9ì,+?›i#ˆ?r¶ í¼<?a³ª‹×?YàOý?"$n'ô±?q'S¾Ë.4FGL J0812.8+6507?ïŽÍžaˆ@@y§~^ª°À:žÌZ·»À<š€ÑK·Ž@ 'Íút@wßÖjÛ?¿kÂ_¥Eä?ŽŸj~y?ÐîOá?@>!œÀ–?î)Ý´{/¿èÜÏ^w"œ¿à'ä¾Ûó[¿ä"¥¡º¥X¿áԦ˱D¿Ë7Qzñã³AGNbll3FGL J0813.3+6509GB6 J0812+6508?óù°˜?xÚd™ºÈ%?`/Z2tU?T.HNåê?ƒRlu<Þ?vš§4òú?îñ™²é?šÄ .›´?c}n—š?mDò=Ò?Ÿ]êZz?˜©KíÑJë?íñPø`—?¶#–Æ?~‡¿
ÂÉ?l•w"ýþæ?­"Ö?Ž	OôB‹?í·QœH)?'l±öX@?Y՗Ä?wü°ÏÄc?¬¸Õ€v̊?'/#(HO4FGL J0812.9+5555?Å7‰àg@@»3ÞLQÀ:þ'œ&;ÔÀ<¼MÑD*Ò@ ž
Lµ@CHÚde?ÃMИ^[*?"V±^ÿŒ4?Ђp½Ø=C@Àõܼ?ê80Èõ§·¿ç_&DÉ¿æ€(^ÃÚ¶¿×ì"é0°¢¿âBÞ¡áf¸¿ïÿ¦¶tFAGNbll3FGL J0812.9+5555NVSS J081251+555422?ï·l¦á?}‰+9Ȳ?OáÅD?BŽÐ ÓÅ?€&âE"ÇÇ?{ìS&Ý¢U?ﮕ¾Û¿û?Ž¡^……K?:jÏ_öÜ¢?K'"ŠïA?ƒ‡9ÎJz?€Î}èêÑê?îÈ»Ó}dÑ?‡Wd勋¹?j°a:Õx?\ó@â®4K?¡É<¸&'?…ë'sº?ïNüwfýc?yÏNæf‡Ý?l@îA‰·?T´ºž0L?'˜SJüÂ|?y°êæa4FGL J0813.7-0356?ïò¬?Ž‹I@0Jò"z–À:Ê/•ïÀîÀ<p¼Åd@!T(Ì'?ú{¬\ë?Èôî~ù/V?Ç`1Ùkì@J¡äÁ¶@;DI[Ë?ÔC¹"4$Ë¿ålüþóg¿µ…(ÞÆtn?·)£dm­¿ßüEá5ºw¿ç$8YáAGNbcu3FGL J0813.5-0356NVSS J081338-035716?ïS‰ÄÛ§?"JVÒÄËç?eÌÑq&ô?_¸¦æ }H?™»ô™?É?'
s›¶×?îX±ðœ?­ú0…Ë{Ê?hœï\©®?t–ó™'?¨ë)d?­m5ÑË?í4Ðowà¯?˜Íéª?'ÇS™H«?pÈ$7S'×?´'-Ñm?–Þàk=Uœ?ëÐlߨ'¨?¡?´cÔür?‡u@îäº?wrÚ1]ã?¾ðäÞÛz? ßV¨‡ÇN4FGL J0814.2-1013?êË~Y"é@*m¾]ž@ÈÀ979_JÀ;ødÏ@ûÃ	€@•{âÏm'?¯©¨|Ø»?©^v¿
R¥?ú±ÅÅqŽ¹@	½Õ{G"?ïÿÿÊPË¿Ú$'óÕz¿áÒ¢dCvw¿á$Øâ"Äö¿äŽî_ċ¶¿å›«–òAGNbll3FGL J0814.1-1012NVSS J081411-101208?ïǑ€A6û?yj?cý?9S6&ø6b?53ÆØïÏH?z¢|ôÿ7?x¼+VLõ?ïA¤â—–?˜C{+§?\#a[V?n¢{èȹÅ?–qwǖ?–ÜxH¾<ˆ?î»Ýª ÓÕ?‹É$7ö¤¸?sLßh¥4?fJÍ"(çg?¡Ø¡¢®?‰y˜M£Ì	?îQäTÐÑ?‰IMyq;"?FFËê6?w¨¾ªø³?¢¾—Xýêº?ƒ,&÷CÙA4FGL J0814.4+6926?ÌBUèd@@C3‡	WÀ<0€sWæqÀ=+ˆlJ«ö@"òÌ!V;÷?ú	‡¶Õë?Öxë8Ȟj?É¡ú{±§,?öD?Àà0?ÿƒµl3¿ïýv¸ÄL¿íEIJ̬ì?ïþä­³,?Ë¢Ú`S¿ââÝ°IßG¿ÄC/ÀAGNbcu1RXS J081407.6+692549?ëG(¾?ÛÑêßu?L‰Ä;ZÅ0?P<ƒß«4?†Pèê€$K?û{y8Ù?îèÎêÞ
?Ÿc½àô?cŸºWgJ?u7Ѹ(ZŽ? 9%5¬¨ï?!¬Ôì|?í|µlæi ?—I9j« ÷?A¡o*è?x£
ÿ‰ó÷?±ò jçU÷?•í°£™È?íÞÅÜBö? éOÈòŽ½?iªèéքy?h"ÿYÒ`Ê?°<yÖ L9? «œ'K"4FGL J0814.4+2941¿á?"hk›@=üGõbÀ:õl‰–WÀ<'@Þí`Á@ ³»Öƒó?þí@ÅÂíP?ÈcF¡Oš?²b["Ñ2ã?êÛª ¨»?÷*&ˆó?ïþР@ý¡¿éËßR,¿Ú¾/Gì(¿Üè'¯qr¿à姏%¢¿Ø¦á€¸øAGNbll3FGL J0814.5+2943RX J0814.4+2941?îÒ®êP'?¤Äqx¬Ó?W‰Tþé?QæÜ:Ù?­Z¨ÆºÚ?¤Šb	"ǧ?íÆVVøÇ?³g¢=˜?'ül̇ˆ?¡~˜ï'
?²ú²&W¾?«¹|ÊNÉ?ís*ɏĔ?—_­hr¢D?z2j¼Óp€?i≢NjŸ?²Ãƒ´¤D?–‹úÉÁÇÃ?åögÓ´¥?¨6dCà?£ÂÀA­s?™&釗u?њØPt 5?©jظÄÓã4FGL J0814.5-2642?áÖÙoêÀö@ªžåXµÀ:Ç!—)|ÑÀ<=ŠV/·~@tÿKû<@a$z2Ì?Ï«b"Y–t?Ó½Éd7
@ SŸºE@\—rÍÒÜ?ïœø^Kò?ÕÖ\îm†¿Ü±,]Vl¿æ«Ý¾â~e¿æ'ÃÉf¿ïÿÚ`‰,ºAGNbcuAT20G J081427-264422?åR&ÂóA›?¾ËàÂã?ê	Ie"S?‡Ýá–OÆ?ÔMåƒ#†?¾¬ tÅ£¹?â•H$]f?ÉÁÒÒ?Ã_faª?œ]ãjAnA?ÙÉ9ÀãÍ©?ȝ—8Óu?詀4Og?¦N:{Ð%?©›Óܒú?'¹ë#g¿Ã?ÇX9̍¦?¢l¸LI3&?몰Äi´Ÿ?™õßsk\y?—)žéd'?JÇ¢&¾©?¼ä/tøÛ?—`]ƒàA4FGL J0814.6+6430?äiÆPÿw@@šb=ú	À8©ƒEW"À<µê28a@>Èáè@Á£n.±Ä?žíC\B˜x? XÑÓFäk?þvk+Èç@/¢ÈÂQ¿ßLVð§h¿ÜgÇúÕô"¿äuð²…"ê¿ãsÉü7ô¿ä¡^E°Ž¿æ%ÜÓ«
_AGNbll3FGL J0814.7+6428GB6 J0814+6431?ï¹#‰Z›?¥¤"EðdÛ?V–ö€Íëq?z%QÆɍ<?}È}Ø8?£¬'x<ˆ?ïz'‡:?Ž5êÿæ#µ?R´EÔ}Ï2?eYJ#™¢?%mbwÄ?ŒJ0*-?ï C"ƒï?"qÅv˓?o¨>üj?f"¿Ñ§:?˜f§¢&?'r»a'½_?ïØÔPð=ý?a¸»£.Y?aA—Þ½¸?S¹{»Ÿy?fmwãE1?VRz[Í]4FGL J0815.6+3641¿ȩ̂çÚE@?ì"F{åTÀ;ÿ!³®ïÀ<˜­4
@-£ôfnÊ@[¡/?Ê_d©ø·a?·oÇäÌÃ?ï2 Ñœ?f?îÅ.S-,<¿áBÓNÇ
p¿Ë@%	#ë¿ê¸¬"Wé¿ÜÕ¬˜¥¿æv¯Æ+É¿ïþϞŽKAGNfsrqOJ 320?îî·ÂvM)?˜xè¶+Áç?sƒW¸¨?€®{†Œ$ý?HB* l©?–tH‰þ2?ìe€9ãqH?²þ'©MT?žx£øŸY?¢/õù÷i"?µ5Õ2ލè?ª2°`¬œ??íSM‹º?˜Y<ׅWµ?'r‡H }b?…·ˆ$KE?±
cÁšj?"	ÖÓÂ5?çlîtà\?¨ú5¸íQL?³€±ú
?›>߃}?Ȍãm/y‹?¦Õö]õ4FGL J0815.9+2951¿ã½S4Qãš@>VΚ,fÀ:ûàÊ°'ÚÀ<q±6nQ@E´%¶óÈ@zvSCsó?Úz}ib?×r2aüõ4?ÿ‹µÆ 
b@Ùèú)ý*?ïÿ~‹¡3¿àLÞÕãÍ¿ÔôŸd3Ü&¿è¤N"áÉ´¿ïþ8µS3"¿ïûÀj¾º»AGNbcu2MASX J08153642+2950218?î…þAÛEc?£ XŒàI?yÛnËB:Â?z3÷š6«š?¤d®ãb?¢¢´‰r­"?캎9r‰7?±[N€®Ó?—ðLJˆ]?
jRßõ?´/{!ɞà?¨èi˜þ?éªèÌ°›?¦Œl´¢Œü?²¼ÝÆ#?˜[ˆó0óŽ?¿ëÜ{ùM
? 2îœ5˜û?çá~¤øûÙ?«-¬¤RÁ?¢D¾ˆ&?—&v¤¥Ðf?ËèÕë¹ì'?©Ö¿^Vÿœ4FGL J0816.1+4909?íñ[ï·U@@Ü!BoçÀ:·HIÑÛÀ<«¿2°Vu@=>ô‡|@-Ðãe–?À×h‡'üô?°åä Óö?ðbE¥%¾Ö@ùì¿0þ?ïÔ\
G`¿×ËïW;P8¿ãGø½Ÿ¤¿Þƒ.ž#¿ÞNy	×W¿é#7r]®AGNbllNVSS J081609+491005?ï¥
ìc?u'Ý!;™?b®Îîܳ}?TÅ9.¸L‰?'Ñ+ˆ¬?s<™LhÉ5?ï@þå+ß=?Qÿ¦'¬?]¢1ôŸò?giÚM1R?–;BÎT?vF¬Øã?î. VøöF?Ž…nm5V¹?{\iadÌv?hמèÒ¯á?©²mdD	?‹Áž6ÎT?íýQçØ-?Š=I¤]¦ê?'_l'-?y‹™'k™â?¦ûc;B´?‡<֗?ï4FGL J0816.3+5739¿íÔÏH/Í+@@ó¬Äï‰À9'—¾WÀ<1áÜ(Šc@Tåÿù @CrSÍÝ?¥ LâÂé…?¬Ò½–gÐ@¶ÖU⊤@¸õh¢UÖ¿ã~É3»o¿ØG"ÂLÁ¿â±ðrÄB»¿Ý"²œõē¿å¡…¡?*b¿à<	›Š4¢AGNbll3FGL J0816.7+5739SBS 0812+578?ïØÓÂQé?j-âêä?B÷©éC©?:Š§¿k]Ö?q7{᮪s?h¿­,c°5?ï+Š 	Û?˜@
ÑwœÛ?e¬qÈÅÀ?všWG@#?—ÙÃz?•ª‡ßœÂž?ï?'W2YR?#ͪï÷?fðÌYY7r?V£_ü¥Ö$?•<ûŽ‰®«?}[¨W¬9?ïa†ä·°?‹×=PÌ?"ás<t5¤?oª«iñüÕ?'£….ï]?yw|£ÿ†f4FGL J0816.4-1311¿åÂ¥ëÑ8±@(> ÿT–À8ŸªúêíÀ;Ÿž¾œˆa@èð!Å?ü®»iÍùó?¥xÜI'Í?©Ñyž–Gn@u¦uJ/@ÆÑÜV,²?ï÷$ŸF¬¸¿Ýƒž›3»¿àŽ¡¹"ËÝ¿Ó禆轿àce•†¢¿Ùf=̔CAGNbll3FGL J0816.4-1311PMN J0816-1311?ïÙ ‰®1?n=U0ì?/R,8	Œ9?3? y*?r5*è›#?m^õ+1?ï‹
óÌ?Žôjû"´?Kƒ_±ÆÌp?`Ñ5Îb?‹"i‡ð'õ?ƒ¢ù¬DÜ?îm†AÕJú?"¶¨"Ó?v-ÚmÓ#?pN½i¥d?¦c¶']•ö?'§œ|žj€?îÔÒeR±?‡c¬Ø®ÿ?hÍñxÊçî?U1³I?¡%ú–î&h?†‹Üdaýæ4FGL J0816.4-0007¿ïôP7-œN@2Å3	AÈ!À;+÷­K'FÀ<y³J@å´Ð+Ò?ãÚPx¾W¿?ß4þúÇ[õ?ïqèEÏ?úΘ´—Ká@帧ü³Å?ïþÂ^§U¿îPªJè¿Áb]åc¿ËÑexTÐg¿ïÿJ=eç¿ïÿÿ>¹úAGNbcuNVSS J081626-000559?ïÍôx? '\OlÁ?n
©ÆB\ò?s8ãU.?˜…	Ȩ´Y?Ÿ½
<]ƒ?í*Ôø2"?¿P_‡¹Ý?'vßÂlâ*?ª¡š0Â?² MÔJÜ?¹gÃâ"aï?êÁa?¤ZÚðt1?©YýÌüÖ?"W+þÞÆ?¿Tù3Ž"?Ÿð'Þµ¶`?è^e`ö'Ë?Â;,cÆwƒ?qµkRäP?|»êÉÙ¨q?Íø¿»¯?Â_ønMI4FGL J0816.7-2420?è(Ó± ÿó@'ܱF^‰À9މÁµA–À;ÒWF7ò¶@1f]×÷x@Š(ãN'?»a'þ0-V?Æjsç-v0@	¯å†6a@ۉ–AJx?Š‹h(ˆ_`¿áU±wÜ°p¿ç8Ò¿€#¿äi+<Ĭm¿ì~Ø;•Ø¿áâiʀAAGNbcu3FGL J0816.7-2421PMN J0816-2421?ìéRAÒ5T?«gqLPÈ?¤Ÿô7#¨1? nÛ¡Åf?¬Ê竹›?£ÁŃ3?í|¼U!–?³Gü³·€®?\Öõ³TÕ?qÖÇ %r?³¦Á€'¢?³'ø"‡Ç?ì¬,ó'Ä®?Ÿì6¹qŠ¼?›aÀ}<?ŠÂ<èҟ?³ÆWa¹»C?˜0{s,…?î+­§Õ4§?ŒFÂÓà'—?†(Àx¨?k˳e¢&?¨ã›RŽ´»?Š7R#³ŽÆ4FGL J0816.9+2050?ËSÌ}>@;»ä›«—À:•"¿e=À<f:N°g;@·ëm÷ªF?û<¹t*tH?Â2¡èȀã?È×(ñ:ë@Öoþ•œµ@ãbý%Z-¿â'úÒD?ïû(Êúd¶?'½¨d-ٿӆ÷ µí¿ãð6(°ù2¿ãÂýuâlAGNbll3FGL J0816.5+2049SDSS J081649.78+205106.4?Œ?°Ìû… è?™É"`i)\?°I)ÏÛ?¤‹ÝETv?–\<ÚQ™?ïMç¼?™Ž3!踷?qQë[R€?€c°.'?˜ÈE¹sû?"†ŸO
,ƒ?í5
Ñ%í?˜™%bÄÕ?"Ûˆ>Íâß?†Åø³TÄ?±`ÇgÓWã?"¡~G"?즼(ÓÈV?š×()†"}?˜¸ïvÅ?ƒçœ"}
?´É^%ߔ?˜Ïrƒz8A4FGL J0817.1+1955¿æojŬÙ@;rÍáŸÂ©À;JžWn{ßÀ<£ô¬å¦¸@!±=®6^·?û'êÊä•@?ÏtOȸ–?·ùÓ;PŽ?ꖎý‰X.@Z_Çæ´¿ïù·FRʨ?ïÿü9¡â=¿Òfý:'￶'êΕyÏ¿é2IÉw­·?ÉGŽAAGNbcuCRATES J081705+195836?ï©;õý+?:©ò;†¦?POÑ?IrÚzã™?ƒ´]±E?€–º_†)?ïr뚩چ?‹V4AFW?SY~F,7?abe.hg?lü'àL«?‰kPޟ?íïpîl[Ó?'(I˘ˆ?€#'I'#ú?v/"ˆýH?­'FðyØ?gxàîf?íˆÅèþ?•iÁÝU>À?}Ͻçð?m¡°Ìu	?±â
ò@oÍ?•@6ëý1©4FGL J0817.8+3243?â'êñÙ@?{y¦µÀ:¯*‰@†À<pê?«ç@ a1R]oó?ý@"Êý¿´?Ï:N°g;x?Èü†c[ïë?ûòˆcp'?ûnºÖ*C ?ïgI}!"¿à–ØŸ8¿Ëñ†ÕòV¿Øx$>x¶ ¿à'¨9p¿éØæZgAGNbll2FGL J0817.9+3238RX J0817.9+3243?í1¯Ý©YŠ?¦^'d`Ë?~¹kA?sÒW!ŽØ?´'õ'sLö?¥èë}?ížU`Ì@m?¦}8ÂK??Œ
ªgŠÎy?Q"i(þ?¯?YYE–?¢Oã3?ìηû?œÌ¼{r?Œ´`½‰ƒ'?€ÙzzRì£?µó´n§?™$ì.±?çõ:©Ïÿ¡?¡žIÿlÅ?¤¹šjQÍ+?Ž¼i»`?Êü®¾+Ž4?¡¾BªÁÑ4FGL J0817.8-0934?é_ÞEO²@,¥hÍJ¡À9÷І•±À;¾Ñ"Âr@«è¦
?þB>ƒÉM¼?°	ü-7›£?Àñœdûi@/ô÷í@	[wÿ@"?Í 18\<í¿Ø¢°=w/¿Ø8}%Ō¿â<a_–h¿ä|PKߧ¿æ"z~K_zAGNbll3FGL J0817.8-0935TXS 0815-094?î÷hIÞ«?˜†ØŠL™h?x)¦Œ>?{£ÊÍZ–?›
lZ¼S?•š—*;ñ?í^ƒ@J?±Ÿ‰©–?ŒqÀ¨',×?–Ǫ¿È<?¯âyí§p?¯Þ፶¼?ìÂzß[…?¥#‹|G?¥'W¦u¯Y?™0'%¤K?®°úhD˜_?‹l?êÕËuTù¾? bœáÒ?Ÿ#ÅÍÆÌ°?ƒ];hÂ?ÀÄYpó?t?Ÿ$¤ê'4FGL J0818.2+4222¿å/[žtl@@²`˜À7µx!yÍKÀ;lðå°Éa@'ä6>U?ÿïCZD?–µc›þ?µ@j~N¬@ ­¸d"@V{Šæ¿ÄB1¨Ä"Õ¿Ú$¡4˜Ž¿â[Ã?…Q
¿áçø¢=­¿åŠK1Þt¿é3
ƒç€­AGNbll3FGL J0818.2+4223S4 0814+42?ï¢?Þû–?§´‡€´?OÎÙ-£¾?fDÃǚÔø?…s'#‰ÀD?¦hw¨&\Ž?î]Êlì?ªûÃ÷ÐW¶?"½\×WW?'ˆãûEì?¥Â)è‹b?§‰@Óê˜?ïæõS{Q?'lwó>–?…ž8ΈS?…7ðÒUî¥?'TîL'á?…Bã•0¡?îÀ/Ùð®&?Žv©s?'Å[*׶?uì¥Rw¢:?ž—{TÏ[?‰°µÿ;{4FGL J0818.4+2816?î­1ó(gc@>là¨KäÀ:ªp-…DÀ<‡ËCòž@šÞ‡	t?ÿø€¯½È?Æ3©Ðži?Áío"3,?ûÂùå3Ì@5½'"Aç?ïÿqÐ&ôa¿ÔÆÆ"Ž ¿Ç¦F{9‡5¿ç骾…m¿Ó÷V
RÎڿ㟟m1AGNbllGB6 J0818+2813?ïe¥t\–
?Œ²îf6Œ+?NͤLøß?Hm
ƒ•@Š?'TäSzÖÐ?‹Õl®ôFæ?ï<E'ý?ˆ:PÚ'Â?I!Ø[ñÀ"?SìºÕQ?ŽÑ5Üd¨?‡c%D®ÈŽ?î¶ëýQ?"ô¿V•¯?s¢yùGÅ?k*¥HÕí?¬€B§2A?"ÎÛ}3?îÌ1o®ËM?‡ùŽHÞ?n\Ø£æ"?`¢BÛU½?¡WzÔéð?†­'|Uê¤4FGL J0818.7+3153¿Ø7ÝÆø«@?vq%Ý	[À;]r{ÛCÀ<´°X"@½ˆÍC•+@‹t"Ì?Ðԍ çìŽ?´˜û(·¯?悬î
46@
½©y
­Ù?î9Xç!â©¿ëL´,j?ڒ1%;ù«¿âg‹_D36¿ã÷÷ˆb9±¿ïÿæ¦SfAGNbllB2 0815+32?ï› Œµ?•Ø÷7™¥??'7—?C,6èËa?ˆ;SE®?"£ð*ƒ)`?ïsÏàòk?"ô`{n(6?Pх÷´y?d¶™×
Q?-¤fk?'€væÉØ©?펌"hÙÑ?¥|÷
õüÀ?k"½Tó‰Ç?d°€ç£®e?²®õz•,?¥BKÕÊv?ïD¾:¨S1?''0æÖ?P?ÞÛ3?G€gÄÃVz?–gt­æÊ?îëÚÂ4FGL J0818.8+3229?ҕœ}f@?žbÜn*€À;.'4ùÀ<b¸®1×@Áœ/ñ	@!"U…?×Â$g¾U;?ÁώÞ§«?ð4Ä}ròf@«Ð9h×Z?ïÀ«÷j/I¿ãÓîÿý{Á¿éq®~-,‰¿à°!/ûpN¿ç&[L
¿ïíp±C‹AGNfsrqRX J0818.9+3227?î#àS}?¨‹	Â
?[ ¿+¸Í;?Wv·F±ž?¬òìjiw?¨;±ÿt-m?î´²Ä!3H?¢Ðág™À?qu,l>
¿?ˆº¯œ‡I?¢†.0e
6?žk[gC¤­?í¨Ü×H?šïRÿŒšÎ?r:+wæñ±?`‰4vµ?±•|éÉn§?š1Ãêwôu?ëíŽß5P,?£úB7üñ?{jÔ˱‹?tɘ''C?¾ÜÛ¹™Sƒ?¤ƒ3Ñ	¤4FGL J0819.0+2746?î|LÚ-Í@>j;šàÁvÀ:v[ËرÀ<y¿¼CÎ@‡ފºY?ÿ'è_ÐJ0?ÉIøÜö¼?Ä`EKc¬?ý&ðš1o?þ¿Ý/ñ?ïùï2b¿ä´Ø"óÙ¿ãã9Ü>Z¿×Nø 7­ì¿èLˊ­n¿ïÿÛLÂPrAGNbll3FGL J0818.8+27515C 07.119?ïKô[?‹I%<(t?m¼MëŸ}?oÕçI€ja?'å—À®"?ˆ$i¸Ù°?í½u¯nœ?§fN31Š?	$Æн?"â5yÙ+æ?¬& }­ç?¡yü¯ÝÈB?íPM`:?˜«áÀ'®N?‡V¾¡ìó?y«šWچ?²•/½ÀÀ™?•3äӚñ?ê,8_nÔ?ŸîíT é@?°^¶•¯w?"­z¿v½?¾?ˆwUG?˜høÍÈiº4FGL J0819.4-0756¿Ô''ÿ¾´@.úò¥µ1À:¸—/\À<igÏòñû@!™9ÍV5?ý?cr–'?ÄG?D8"?ûžû?Íi²KAG?í°T¸'×¥?ï³~è=k›¿é°iS¿å XóÖ&¿Óˆ!Äuæ¿ÖM
ú¿yR¿Ý¹žrAGNbll2FGL J0819.6-0803RX J0819.2-0756?í–;ýZ=²?°5ÆC1–?`ºûr­?[EÈCii?²ÈOÍU.Ö?°)ª@‡^?çùŽL9¸?ʛjŽd?'L R4¤U?›÷Íí"÷v?ÍÐBÄÕ,˜?Ê6«77ӓ?ìϓö¼.h?ž¶Ú–ƒ?€p°kã/?qwé‹^?·uJ<¬[?¿Ѐ9?ã9?ŽR?­3ôŒJu?¢¬ÁŠL\?'/gQv»¤?×}õOš;Ü?®+R)£-4FGL J0819.4+4035¿ÐºÜ?0—x@@­UÅ.rÚÀ;ZÄ"ðÀ<ÀëóÁ{@ xE×Ћô?þ©Úª!¨?ÌÕ2÷Ï
?±:‰hÉíõ?áDø®ÖÃ@<pŸû2'¿ízÝð,¿âBMb3{Ø¿Þl~Q¿Í¹±<"›¿æ²"L*zþ¿Ý1a¥1'AGNbllGB6 J0819+4037?ï¬éÏ/?tŒ8XÅ?BcõôFG?4í}Ýt?ƒÓÆ,ø°%?t[•îˆ?ïv&Ь?‹Fº/ñ®o?EOÂí†6¢?R2¹ÕCo[?¿¯ÿø£?Šő¸l?îO'ŸÒQ?Š˜°Ë'àˆ?qg–ƒ.R-?]n¤Û`¼?¨Ùì%³?ˆæo>,?{ç[?‡6zŠµ?ew€ä]÷?Upg'äî?¤W%P3D†?†õWùâo4FGL J0820.1-2801¿íöKêAÛJ@ä—t%kÊÀ;nE£x?­À<ŽOËð-û@#'Òëò_?öø¼ßï¿@?Ñúj>ã¸?ɒOù<—`?÷—%¶rî4@á)`Ìt¿ïÿþÐñ?ïþ!xöŒ¿ïÿã_¶Hý?ïÿð`OËð¿ä2M?Mó©?ÁcÄÄÂAGNbcu1RXS J082021.9-280206?ëvŠ¹·¡?¿§ªLVÖ?a{;€öv?_;¼-:—?Áßè-ÁG¢?¿z£`¿}?ä᳸?Ðw¢¾¿?‹I°Ó±þÔ?¬f(#n…?צ·-™?Ð2Ѕ?èÃøzpή?¥cΨ
p?Ž¾hü"m?zÐ5·ê£(?Ë5¬ý?¤«ŠM¢T?ê‰v'7?µõª†÷¶?'>F'½ƒf?šãÓk9bj?Ô'ϲ¶?´ì=yc÷H4FGL J0820.3+3639¿îeìzßf¥@@l% Jù#À:,Ú"ö¥
À<uo·HJ@Š%»üE
@"€Þô?¶èô˙q?¤Òhÿ./$?îRœàKß@½½"J¥@¿Ïœ¤ç€'¿áÁ÷Tð¿åùéÀÎfÖ¿áyPFGã¿ånbHÊt-¿ç!ñ¢DõAGNbll3FGL J0820.4+3640MG2 J082018+3640?ï^éw?Œ}uÅÄL…?hÎV½‰*º?['»~Ýç~?šcIKù5?‹)^Y{zÝ?ï\›ÿxB/?9ש›"@?XÅ®\?d(LûÎE?'â¯äœÐ:?Šºêð³«?íïÀ8¡ÎK?'Ñ÷1Ȕ¬?wHÚ%i?pÊæ¡¿m?¬¦*Rl'ø?m½'
}7?îE­.(ä?ˆíÑ֊?;\j¢e?r\~%‡¡‰?¤VVTØy?…Ô†T¥›÷4FGL J0820.9+2353?"ÐñÝ8@=ŸÑx-8GÀ:ÎQ1JüÀ<yôÆ)@¬K&ÄåÎ@l#ú±¦?¼¨ñPdÇU¿²†æ¹‡÷?ô?I)>¾@5."hƒ¿åñ¡mx~¿èOÄÎщ˿äÐà,Ðî¿ã ÷&<ª«¿àWg€桿Λq ?[AGNbllGB6 J0820+2353?î½$*œ?–³,eÏI°?q8¦g¶R?eÔ=*ý‹?¢
çð_‡?•5œw0y?ï]îAy]á?ŽûŽµÝÃ?Rd¥ð÷
$?\£/5²Ò?"íqÄÓ?ŒìƒÅyi?î
½2ý"Â?' ì<"z?zÁ ½0p–?g1"~ýO?«Ì¸¥Ô?'
æŒM?î®\É*x?ˆèY­ÖÖ?qAFPŒ1?bR5ùMÂ?¢üÒ
£Fð?ˆñ´©Jv4FGL J0820.9-1258¿íGàRÕSÉ@*X©XS~,À:z:iˆYÖÀ<^ߘk¥@֊þÌ#Z@ɀ¤Ö
¾?¿3~݀¤? ÅoôZ?âObcøM?üû@}ž'?ï×.Ož£Å¿àA0íÕ·¿ä%"S·79¿ã%aE•6¿ÝrqÂ:!º¿ïûOyxAGNbll3FGL J0820.9-1258PKS 0818-128?í¼z±÷æ?¦­O‹'ˆ²?yž€÷Ì݀?q€Ö¡U·?°'B`Ä9?¥ÎdJ>#?érM5Ë?ÅäLÌD?"iJJp?þ?Š'o—×ö?Èñî$$Ñ?ĞÛvâï@?ìf%:‰R? ACmô}©?ûB*LM?{˜^3ße?¸ÝÃq»Ý?6ÀîkêN?ꪋ%BlJ?š®Yì¸Þ–?ŸPi'ª¦Ö?†"s­i4?ÁkÆFùþ?˜š¤¤;4FGL J0821.1+1007?ï_RÝá@8~»˜Çâ'À:ʺ?+ŽúÀ<‡Q\&M@4êÕeM@…ôäC?ÀxD_U{¿£*RŽîù?â†i`Á¶Ä@
SÉÇߨ¿Þíӄø¿åSŠS«y¿èœ!3Vo¿ß[º9¿ä¢aôçž	¿Ú|=&|AGNbcuSDSS J082054.81+100609.4?ïñ•ÈRªÃ?Q´µ72¯?5uÎ^¥;D?+">ƦÇ?WvûÃ*C?Pƒ´"9ˆ?ïÃè•Ÿ?}¼w$èÏ?6½jHÌó?O*5–Fô?|Ò5«$.?{æó곂?ïCÓ$,6Á?zÇÒô'.¼?c¡v£ä?Ý?Mtü~å5?•l¥ü ?yþ,f5?ïϚ~"T?`!ÿÀñ0î?D¨ÎÀ/ä?2
f!Mû]?u¦åÐ?^á8ÏWUò4FGL J0822.4-2630¿Î:¢™®£}@ãS÷ÎÙÀ;
1'rƒ«À<_")P@0<yûš@uØå	µ?Êúv=Éå?µù…½n¶?îÈ.ØZŸ‰@kk!ŒÏ¿Û½*,ú4?ïïÙAOU©¿ìaÏþ°t§¿ÑHdà
—¿å!){#ŒÍ¿ïÿÐ/WÜ`AGNbcuNVSS J082236-263125?é¨þh:ò?ºƒ²¤ÜÝ?u"Z#±fÜ?r]1ƒÚ «?ȯdµA‰?º]8ıòØ?æöÛ"LI?Ç{†ß9À?l"Ñ(op7?"?ƒS0l—?ÑÙ"žˆ?Ç-v$7b"?èùßF^Q?¤¬æUcÂ?'nü·0þ?vËqüH"X?Éê£O «A?£åo¿¦Y?í]Á¯â¤?•@»j	|`?ŠÊ³ø…nƒ?z½=4ÂÝ?±¸œÞdþ?" mè£Ë4FGL J0823.1-6330?ͨáñ;À-Y± žÛùÀ;¤öL"'À<¿';ý@"Ùa…«ü?úaAcwž?Òæ">eìC?°=˶¶¶?Ý¡faÞÂC?ý¤¬	ˆ¿Ø¿ïǃý{u¿èó.0D?æ/ùø??¾îê.£ˆ¿é²ò€»|B?Ùã&2ƒAGNbll1RXS J082316.0-632928?ïnøâɘ?ŽXÈ2Å:??3/†ø`?7²Eêó¿#?'¤èŽã:?ú‡LO>?îÎÝ|dë?°±`/áfI?KälB•Sn?`õœˆ^WÂ?¢¢–ˆ¦ùŠ?°¬;qs˜?íüçH°ƒ0?ŽÝ'ä _Y?t-–""J?nÔúšŠdð?­¯Â%Zd?$=QIx‡?íW@»ò9Î?›" V(ý?a#is§+2?`–2K¸ä?´¼ÞÔÐø4?šÌøK*"4FGL J0823.1+4042¿ÐçéçBw|@A
CނØÀ:K _ŠÀ<S½—¥£"@E§håÎ@Ľý&0ì?¸ÛÖÕå$]¿˜Ù·–Ú¢?ßi›"Ö>@KÖWºüì?ê_ëä¿è°Ô^;Ÿ"¿æ†Û†£ó¿çÞavؤ¿ÒB&€IR¿ïü5ۄµAGNfsrq3FGL J0822.9+4041B3 0819+408?ïÛ³<kù±?lñÊ'«A2?P¤Ÿ՚ô?I¨-_¬?kút›?h¬J€ÂSO?ïÃÂÄÒh?|é ð}£?4µ4SK_?JzšŒ¥?|ÓJQ—G?{l§~°Ì?îú35iq?ƒ4FöiP?j·ãÊv¨«?XÌZxÄ:¤?bœâÃüË?'=Š¦¿x?ïËO'l?b¼í>ÕB?>ÝC@/ÓB?183e!?xj˜pÌ-?b}†ôÚeF4FGL J0823.3+2224?îÒÇçF@=­gf@¦¹À:q(•J€À<rv.Z†^@yðÿ±üg@#Nƒñ'¨?Á±=òÕ?º"»¼Pí?ö4ƒzsc¥@q,/³ÌÌ?ïªì¨4g¿Æèž9'q¿åèº3mÖ¿å*@ ¯¿ã5ækÚ¿ïÿàŠï²«AGNbllOJ 233?ï_fL›åÂ?…8pg8sO?jWœsÝ9²?aY(/€0ñ?ÈBÞ ™?ƒD…"çb?ï?MdÊ'³?wû—»¼Þ?cȌW*Œß?köƒ>"c+?•AÛÕ¸#?&	~[?í‹@¢n ?"ÿõíº#(?Øþj(Ì?yi@6Ï6Y?°ÄÛEÙ?'%ót"cì?î'ŽsîÎ?ˆs,º–R?—/ð"DrÀ?~(Ýué_™?£îÞ֞ÙÍ?'ª=¼àé}4FGL J0823.7-4838?ÎÞé~xÜÀ¤B"ßÎ1À9GÙ.ÚÞÞÀ;-‡É},@'¶iÞì@uò£ +?ÀAž0O‹?±j¿ë½Ô?ñj µ'-l@ÛW‰Ôª'?ëGU^×%ì¿éfA·/'¿è¦¶~¡Ç¿åýÃÝéU¿ìÔ
xÿÆ¿ïù·KAGNbcu3FGL J0823.6-4838PMN J0823-4837?變˶{ô?¿=hÙÔ?—µ§Gܲ?(HJŒ?ÊbÞ=?¾ªÌO?áÌøµ«æ`?Ëø&Þsñ?''©?C9'?Œ\ö±G?ÛÔÑJ®w?ÌY^)È?ä­`siP?±é'0þ*?¬?OØ$K?—ƒëÓ?Ó^/2[w?®ò†éË÷Ì?å)@Å×ô?¬(jã"Ä(?©%é?Û?ŽàÚd|3˜?҈Î+L_Ý?¬—,,Š4FGL J0824.4+2440¿àŒ.Á"cq@>¢v§&JÀ9žØ:¿¯À<û¶Å#‹@k"+'s@qý"ÕíÞ?°¢"hR#ä¿¢…>©€d?ðÑ}†=œC@!BԐæm?Âcþ"8¿åâX"ÖÅ¿çñâÀÿäý¿áÆýX…Ó¿ç¹û~»òµ¿äGDžkAGNfsrq3FGL J0824.1+2434B2 0821+24?ïí5~h×?WŽçSЇ÷?A:r§lT'?6JCdç\Y?\÷Éڛ±?TÕ³œVž?ïÅÿ-ø|Õ?|Œè*¡²!?9/œúNc­?R*Õ;	õ?{mo4¯Î?z• {Ð÷?ï'šüOW?€Ø
VŒ¿¬?jþ×&|J?Vn29'?—¬Å"w…¤?~üâʆ¨Ž?ïíöiˆÈ?Líóž÷É?1	‰|çI?Em­þÄ?_ќÍÊö8?KÛêÝjy—4FGL J0824.7+5552?Ä­"êžC@AüPHÀ9yú Âî'À<b[ŒÐ×@ŽWáé>@ÀY+",?ªæ%®¨?ž½»"GoM?î\fhå@͘îxîÿ?³ÜÝf"â¿å˜ËЮڿç»ÉÚª"¿èœm¿ ;à¿å(œ×;»˜¿ïÿ±'#áAGNfsrq3FGL J0824.9+5551OJ 535?ïó÷Q=V8?VI¾{(õ?1´ÉÔø­?&âêÅ?C#?S¤VÒÞSù?TÿóaßË?ï·(Û"?€ë¨ ¨Ò?B@yAè¡'?Y±Hû_¦?Á£[°Û?|Q—dg??ï=ÃÇ=2ã?~ˆ"ˆZ?i£Ú%¤àK?Uö›ÊùôI?•Ó¥²?{Š8FãÁ?ïð6 í€+?M‰Ì–O÷"?IÕ§:©y?<]¨-@"?SSQbT‰?EÅhBPa4FGL J0824.9+3915?ï÷®LÕ`@A¦ÊıÀ9'ÛçòÃÀ<Q¶¯T@ü¦–WDà@öƉ¼­?±Ï	¤ïc?º@ÂèÈUð@fhÝ9+›@˜q±CÞ?î¤vlmçd¿ÝM'iÒ,¿ç–ŸV¿äq¦ ¿ç¿ëÙ~áÝU0¿ïÿÏù§÷*AGNfsrq3FGL J0824.9+39164C +39.23?ïÁ¹åž"œ?vözê/½±?]âÚ ?U4v}QR?wá,î¼û?t_ˆïÌ?îõ².8¿O? ;6{ɲM?w	žm+?‹ã}A|¿è?›‡wQLË?–ó.ì-¬g?î¸Qûëµ?Ž.¨>–M?"KÿR'¹?}oáL÷Ÿv?žÏÐW9,ß?†éüwÎc?î–=‰GQl?¤‡dÊÂ?Ÿ'Kl@û‰?‰žv§^?Œ"Õ©®B?t	2d^Ð4FGL J0825.8+0309?ÑFàM¡ã.@6c¾˜V£{À9‹¶–ç8À<>æ¾æZ=@쮪ì}@œ@WV?¯_8ÕX7¿@¢>ͨç?'i1qçú?ûA7ë~¾¢?ï7É
ûk¿äÙ¸£J"¿ãœ
!Áñ§¿ágFáúÊ¿ã‹= Êei¿ÙoÐ<ÃÕ­AGNbll3FGL J0826.0+0307PKS 0823+033?î™Zžì¢Æ?ž›;p›³ø?t'£©Ïy?o㫌n?£åa›ûñw?œqN/@|ø?î[õ¿Ì?¥›?[¤ïI?"fºúx{?"ìD"òI?¥&õP8ýè?ŸÌ+" ý?ëªûã—-?£tYW9(?•ÑyøÃǃ?"F†÷ö'	?½3Ȓ²T»?¢
•ö걏?ìèµFö¤Œ?žb2lÝÏ?¦ô?Çîj?'Ÿƒ«ª´S?ª€kȧ—ã?'f@{˜4FGL J0825.9-3218?ç«P‹]Á§@
tO»)6ZÀ9NW±—½!À;¦€ç,¬@"­K¨@ºZÚA*?·ì
µÂÅ?Ï£Û¼Ô²@è&grÕà@wT©¥€X¿Ù߄ÊÕ{È¿à"b*—ƒ¿éE½úL¿è5QGq¿îÐîdÍ	3¿ëÓb}£™ÎAGNbcu3FGL J0825.8-3217PKS 0823-321?ëðJÆ?¹¢šîþ?²U»Ä'}?°MÅRV?´ÂÁêíÜÌ?­G¾ÎöŠ1?ìыülÖ?ÀJW‡+ùÜ?{–"³Ð?'üH§@?½*ÛÆ%˜?¿â€dúÒb?êHÍãzØ?ªž&êúl}?±LñÂtŸ?ž7@!·T?¼mƒòA´›?¢/Ûaý"?íNlb>?'W¿+÷Qž?•5¦Tt>Ú?~uTČ6?°?3Xòð'?Éi§†ÄÜ4FGL J0825.9-2230?ßO֍ڍ@!ÙöD•[FÀ7ތXhvâÀ;J	{¸@Ô{Aê±?þŽ&žÐ:@?šN‹9•´?°…OŠ¬Á¿@ÿkã}é:@Í+Pæ¢a¿£ãŽZKP¿×ôsúù…è¿á¿6â]¿Û@êa2J¿äšÀá@¿åuÀ –ùVAGNbll3FGL J0825.9-2230PKS 0823-223?îÑn"Þè
?"y[ñüž?Fµ‡ÊÚ©?@ߘÓÔy‹?¢ŽA"
S÷?"YÖHϜ?ï?סÉ4?¦6ÔWÓ¿?b†ù`¹?xðF³Ú.•?›£:ç­E?¥ìW³ão?ÁÜ{t?"L9†*xP?€¨Ÿn}V?xøìüÝèµ?¢ÿ™º\©h?Â ‰YÁ—?ÚVz?uùZ±k£l?T9_w²?ClîáÚ
\?‰Ä]{|?u~LÖ¶¤d4FGL J0826.4-6404¿Üó-äê¥ÑÀ-XçW'Ž
À:‡‡H^>À<='JSá@!ã~êì?üqšânõ?·SÈ)$?œ(b}VK?叀[@áäÃ
±D?ëEKß&–˜¿àȳÞq!¿Ò•½Áìõ¿ßû[O¿Ø¡ŸAÏ-O¿ÌŽ9G¡AGNbll3FGL J0826.3-6400SUMSS J082627-640414?ï$8r×ø?+2š"?W)j=ã˜Þ?JؼMþž?œÈâMÆÇy?~¸DÕJo?ïlÁ]À›?T.}r?D{³‡Æ‡?T™äÍ5ŠF?'Ä«®œ?ŽyЭ,jœ?íƆ|+™?–Þœª/šÿ?vËø¯º™y?lÀŒ??°_"«¡ª?•"Z‰Nß¹?íIÞyMYq?"X4ïZ4æ?tHGiC¨#?a£^‡÷ºH?´l‡¿ùò?"Nø¿€4FGL J0827.0-0708¿'}6F	Ã@1† yKÀ:¼gú»À<5m%H{@ ®TL2ˆ"?ú݁5ž?À1xÞc"9?Ãúr¢^å@7ßÖjÛ@ûEá`­•?ïòMZ%æD?Ýêßqêþç¿ÂÑå:Ü¿Ï÷ ÞFò®¿ã™:Ü¿ÖElÜ!SAGNbll3FGL J0827.2-0711PMN J0827-0708?ïL~KãC'?ÿÖRÚÄ'?vËÁ¡Ð'ó?oÿTã?½F#kr?Ž¡É‹*3À?ï!Q–ˆ_?–Ð[ŸI?lŒ³c?wÍèÛ.†?˜Jßm+£ã?""E^Ï?î6Тˋ?"N?ò¸Y?zsú'Ž¼?qVeh9ғ?©O³³õ"?"P_|…=?ëäJè"¬†?šwT?òÌæ?š?Nƒã;?Zë0%H?ºUØëI¢ÿ?—÷§£q±	4FGL J0827.6-3735?àrOßÚ?áß®PàÃÀ9\‰Õ×7ŠÀ;-«‰†&@ŒhF]0@ì["e…–?Ì,Ë:%•¼?Îñ¬€&+
@%[Új@
±´Ãk¥¿Á«w½{Ëþ¿å`=Wyc™¿ìD‡•¿ïýÜ¿‰k?âɃ¡àø¿ï¶1J$ç@AGNbcu1FGL J0827.9-3738PKS B0826-373?ïf怷é?š‹2¿õ³0?\Í=sÐat?d$΋A—?'V\ÅÙq?™'QgÓÈ?êxøŠ2ÜR?ËyPÞqÄ<?ŒNõ[Ou?³ÝÛ#öD?ÄW4ÇÞÙ½?ÈôvËâG2?år4kÜÍ?°þG£¸¬í?®Á߃?D"íË+R?ÑCs™V?­ÜÅäC?îóRò¾t½?™!"-Û	?=Úeç^<?BöKÏ=fŸ? IŸLåh?˜ùÏlü?4FGL J0827.8+5221¿ïÑËup@AÔîàóË>À;Sx›ó-À<¸[j‰á–@ ‡%["5.@µPy•T?̊›9ÖÚ¿Í¶ùôº?Àvþ#±àã@¿ñÇx?ëKå±  œ¿è	cr– ¿è]ÕÉ ¿Úm¾I|K¿ß[ÿDÄ*<¿à]¾÷÷ôAGNfsrq3FGL J0828.5+5217TXS 0824+524?ï'j:åN«?']ïU¡@²?[Sïü:¢°?PrdgÅË?™]y£'€ž?ïY}"£C?îÐed(ß?œ¡I4Báó?fé™ÌöÆê?v¯'òߥ?¡ î¢?™¹Ë*­¹?íØùk'?"!êo?ƒ_?tµ`ìœhè?`p¤Ð?¯èäReºÊ?'ø£¥‰¶!?íO¢³¿"M?›š
·è?uU‹x‹¤ˆ?goWS¾µ?´-'ª{#U?œ1Vlê÷4FGL J0828.0+2307?ï×z()@>ﯷéÀ;
ê0ŠâGÀ<Ÿ	"5"@ ü¢¥‹•?üÉJç"Þ÷?Çö·ÂN™–?¸'ˆá±O?ñØyÞé/@~ç­Î¯Ñ¿™ª8€Ø‹%?í¨ÊߌÂò¿Ø•Þ#6eî¿âHdóŸŸm¿ÉÞ¶Ö:µ¿ê³
¹—eãAGNbllNVSS J082801+231215?ï•Ö;£û?7¼¸NT?V{
¹ú	?Qƒ^ù.¦D?‡ÇAµdÂ?€+¸LìT7?ïqUzO®G?ŒsäXÀ?Sa/zSÖ¶?`~+§±ší?Ÿ=¾dù»?‰£d'Gh?íè0"!?Ý?'±"½?'?yÿH"mB?mf©±§Ò?®=½™tŒ?'/Rf!?íœÙ¹Úô?•x©°éò?†*]ölª?y_Ì°°è?°Sæ‡:ZÍ?"‡݃¾$4FGL J0828.3+4152¿ï÷fÆ|7@A˜©Þ‹;2À;›ík¨Å‡À<â{s=å>@!6ÛìOt?ýÖ`)5ƒp?ÍW³›"…¼?˜';½'v?Ιë£ýu·?úYC[öÌ¿é|O÷Æ¿îEÌþJô?Çg_	й@¿é&b@¼ß¿¬ÖI"]Í濸%^^Z(kAGNbllB3 0824+420?죎?¶?À®Ëíj?K=œ¿¸?Iu>«]ï?º­ÉÅŸ?Ã%´Ž~?îT%º‰ôp?©I/V'?xQtr"y?‹ïÿ¾žÁ±?§³uÉiØ?¥‹dàVÃ?í0ߖcç?˜.¸gÛ\Ý?|DÝoúj•?r]î®Ì?´ºÓ,M:#?—hÝÉ*aÙ?ì—_}ð…5?¤ÜA•²€?^k}§ððJ?_M
B·ð?ºËVÜ™?¤Ðuð_W¢4FGL J0828.6-0747?æ*ͳýs@1‡"%RDÀ:›ÇqC9À<l_˜ìËp@'ÖÃñ†ë@;™ÔQüL?ÔÖàâXz@?ä–ëip@µV=ú6'@èHÎÐÝþ?ïåÃ=×Ñä?>ê!¿ëÃÏ,ù]O¿âËñqÇÿå;Ðá.ƒ¡¿åIßG"ÔAGNbcuNVSS J082854-074854?ìØ{Ñ;ó?°s74"¹?¯ŒePU?ª'q{XSû?¢ëéçð?žÓV=UϾ?è†xñE
?Çìc%&qÆ?À§Õ+Ҙ­?ÃÚ?µ~eŸ?º|•Ц<?³UŽy­Ñ?ë^ÐD§3?¡Ç«žtÀ?§E£ aH<?"
çÆâx³?¹f¬
•Âû?š¹"‹'?çÚI×]á?·jTZÍo?Çv,>ñz?·Žõÿá³?²A[ÆÇ.?œ/}ú·ÄÊ4FGL J0828.7-2422?å4ît<h@ ÀîIõ˜À:̹-³—rÀ<\w—|@^Ù<å@
¥³Ú?Å¢7"0?šP¥<˜•@?Ö¡ô›<@f
#‹?ïÿ€³ï†5¿ç¼"¦Ò¿æ"
q¿Öž:}ªOÊ¿åïŽÎd|¿ïÿz)5ÙAGNbll3FGL J0828.8-2420NVSS J082841-241850?ëh<ÊIpÄ?µeãQXHÊ?jó_²'1?iH¥á¶»Š?Áó?XÌO?µ«Ùá'?å_ô¦öâ?Å56»í?ho†Ó$K°?t5NÞ 'Ê?Õ a	ɦ?Å)P5'¯®?锌Úñ…·?¤~Z\¯ë?Žº4æÆ?ukaÊ>?ÇÂ)E͇Á?£'Õ£÷]?íý*'Y ?ŠuU£i´?gí+[î?eõ Ÿ"¤¤?¬@Z1Žè;?‰]ó—¸#4FGL J0829.0+1755?é¢Eàl<@=]Ù©T"À:pÓ¥¸À<t3Øt ¼@¸ÂÒ¢ú–@7·&rZ?Á=¦©¢{?¹õeó#ù"?úo|—@‡sÐÝ'¹?ïä"pB]¿Ü•)<ºEŒ¿ãðís5Â¿ÞŒ~þã ¿ê†-vZÐ0?™BüÔÒTÌAGNbllTXS 0826+180?îq±M?š=Úe²?†"Š•àg—?€ßoTN«?£^lÿs?–æŒx¬O?îÅ?Utœ?—¶lõÏ(H?sOp³˜¹?zŸxÇë›H?¡B'§Ã?"b6Š`?íPZW?ÌY?›+µd‡ßQ?'|à\"?"z0)Xš?±õ.û˜Z?•]¬,úÕø?í
ÞØz'@?'Èê;n?œ'^¥®Û?˜ÄuuÊA?°lq'ÀfŽ?ŒmQd'$4FGL J0829.4+0857¿æýÖzJžà@9ÐÉûa4ÎÀ:ΖãܳËÀ<'ñŒŸ¶@6"1Rˆc@‰ek"¤?Á€¸HÜ=¿] "øáL?WP¸˜ý@PeAxEa?ïõ+Z÷[¿âH^=¢ø¾¿àÖCnÙÒ¿á`{jÚin¿ßò)é•ö¿ÕwyÿJxtAGNfsrq3FGL J0829.3+0901TXS 0826+091?ï©â¢¿¯?z¥ôéO…?V7–é¯?Ljåë ?'Àdròia?x¼5"Å™º?ï6DÀï*?"iE'†‡¤?[ˆbdÇ`à?dxEТ§é?›à±A•¤°?"`5QÀC?íýlÑõÈ«?WñQÜ«ç?{J‹-0î‡?g³º6+Ñ?¬¿ázýW"?ŽC"«a‹%?íþԎ#l?ˆ2jB#?z/Gb¼2?d)ÔÔ%ãá?¬Ù	ÊÚqÜ?ˆÓ-
*½4FGL J0829.6-1140¿íüúíÐD@/T)¥ë·À9ÍRúxׂÀ<9KWí&ß@Åq%\0?ÿÖeÒ°?µ–È®ÚôX?²†8—·?ýÄxœÉÐ@K¬Ñ¯µ?ïÿÿÊPË¿ß±$ûŒÿ¿ãì@§Ú¿Ó¯ÎD¬¿ã‰u_'®¿éÚ~Q1AGNbcu3FGL J0829.6-1137NVSS J082939-114103?ïg)÷1þ?•ÛÅn6íå?Tõu0%eÄ?O|¹uj"h?'ËiÆÚI¸?•w^lQVÄ?îÞ½3¸µ?žêÁà°Á?hÄè''µ?u¨lQî;I? Œ0uò.Í?0¯+]XÂ?í'.z©Ý?–±6‡Œ?'qÂ/?qá,Ž·Ý?±=|xÏ?"‹ùŽÑž‹?ìœ,Nґ§?';©i…ùi?—ô{è!]ö?zDî
Ÿ¨?µ!~cH?	@……¿"4FGL J0829.7+5105¿ÐÏgÖAÚZ@Aûd­ÿ',À;A³àl½À<ÛãÛÝ@˜¥ûý'ç?ÿµA*l»?ÎK`æõ—ò?¬øƒcø"?á!aRüQ?ûZÈΪ¿æv!ÅL¥Ë¿à…'âr%Œ¿ä¡‡¿}¿ªcÃ|t£¿ïÿ"Àh¡?ïóÕðaýKAGNbllGB6 J0829+5108?爵À$`?ƒž¦Ù Ñ?U×;aofÎ?\®#»Áïž?'h'û(?ªÏÄ^U;?îàìL/?œK3N?=v?hô"Üó9?sðØöBý? aõ½pY"?™³A£!•s?íCß±·ç?˜?z8d?Œn•¸š±?€€¥C}¤Ÿ?²S/»0*œ?•i³•+?î""G'K;?'Z±O4ó?€§>{ã@,?x¥ãï?¢¤èâ|:?ŽþT©v¼4FGL J0829.7-5856¿áÜ·jSËÀ'÷¾æÀ9Œòã·ÊÝÀ<<ʋ©í@J€×¬@€Á@§ü?µØáò½'?³HÐ(ví?ûˆ5©/8Ó@éI&÷ç¿ÔI":<'¿å§zޢ߿çÖj¥Gá¿æ¯qr3#C¿ð?ïÆ1bM§ÿAGNbcu3FGL J0830.3-5855PMN J0829-5856?îü€Žåõ?+F®•Øç?z`¿¹b|?¦ê½¸fW?™×¾P*»D?•à{ԑi?íº3Çøq)?µ£Æû˜k?Œ€x¹Ö=
? g*>1?­<¥R^7?±'ÀHˆ¹Ó?ìO2mà*?£²\@¡xÄ?™KpW±û?êáGu-?·3{:B'?Ÿk1éâ€?íÅ?"XM?™ï\`¿kÖ?"ãâ×Gz?†³½WÞë?©=š¢6ñk?"ÚæµòžQ4FGL J0830.0+5231¿ìœ·…+½7@Aÿz¢]zÀ;ðG%XÀ<¼•¹:I@ žBFK"?ÿƺ~ìo*?Ι>ív?~r‡î¿?ªDOÿáeû@ÍãùI¿å -à
¿ÜÜ
œö›R?îÞ!¯é¿ßu¸ÿ:ˆ<¿ìwÛ~kjÝ?ÛF.b"óèAGNbcuRX J0830.1+5230?îÚ${€†?œ†hþG‰?are9?^ãºxÜrÃ?¡F—«uÏ?›KÍRM—?ï?äü,ƃ?—Ô´ï?`Íg)û;?q¸Vk«p?–&́ð<?"'hû{½Æ?ìã"×E².?œ<˜/½?"±Éìmú›?†ç3s¦p?³öæʶïç?—µ!ÃÆÊL?ïèäϓ?‡RÜâ	?d¸Qöc©?b.ÚÌxñ?š,sçA7?†úœÅ›ô4FGL J0830.1-0946?ص™Öf½@0ÊFà!qÀ;A8"ÀõÀ<©!6±m@ ìcÎ[˜,?ý°áxÚ?Ìh´‰ßè3?£ý?[_¢'?Ü:…M\T@?%ƒr:Û?ïÿùSt¿èýÒ~<›è¿ßŠ'¥aMù¿â9gàd`¿©¶I¨•Šì¿àÚ¡'µ AGNbcu1RXS J083014.6-094455?îäI‰]K?¡©Ó´(Þ?F†[ñ\ç÷?H8¦³á`?¡aMúeÓx?¡|š& ?î2]gäS?·%:î‡n?Y—££äà?p»,ø3m?¬
q´›¨?¶ÆªöQà¦?íK'àWP?ŸOٟæX?jĤN¨9ç?b <‹Þ_¯?´Ñ1žˆ±?ž¾ýƗ"¾?îñU_"˜?†µE8œö?CëZaï?@Ve0k? Ÿ]Aº2(?†¹>ÕË[y4FGL J0830.8+2410?à_>±ºo@?ÛøvžÂÎÀ8´wcä¬À;܋Hþƒ@ÿ).L™Œ@L±:?¦SN† Ã"?À³Eý9@ù/+f¶@—Šh"¿×ÔÁû¿ã9[e¿æà›$´¿é:귙^á¿ì½Ú@¨¼¢¿ïÿïXzAGNFSRQ3FGL J0830.7+2408S3 0827+24?ïªf{5‹?†ÿülóÜ?uÕEn#?wpd€ú?t÷¹TB2Â?|u¡Ö'ò?ï¡¡â.Kš?‡_Ó
óA‡?KbCy¬?[RvœÿT?…ác;d"?†•mG¼|2?îßú?'†ò…{sŽ?…'ÂVOJÃ?€!ô¶²^/?™s¼'xC?ŒÞh-š?b?ïøÎ`pÁ]?=èšÀêî?%mà¹K§Ï?ÕñO ƒ4?Gk§¨$?;'*âÑì4FGL J0831.4+2631¿ì-'Åjü@@ZŒÞ 3èÀ:یwr'eÀ<r7€ŸÍ@í5eèg2@+Iº?Ê°9FÅ?¢ô¤­Ï?Öin¼ó¼@ëpõ3s¿ãà]¾!8_¿áË¿¹Ó¿ê'Úgê¿ÞØ|ßy£¿ïýĆ­-Ë¿îÍ´Þïd&AGNbcu3FGL J0830.8+2629MG2 J083121+2629?ïdýË·_ç?µ_E1å:?lïs™p?y_ ªŒó?"ÅuAª?‹(ö†Vh?ïPÎÁ×ݳ?½ÑÔm(³?X­è»òë-?ed®‹?"[I9Eè?ŽðÄj\ߖ?íÒ݄ï
‡?'£}º%'?†p¹êÿ_?tfáÚÆNž?­5ù6O@1?Ë΢ýß?îÑuàsÊr?†"§×Ó?z­Ä¥‡íq?eØú;KŠ?Ÿ%ÒÈ$¶v?"QíX$ãä4FGL J0831.5+1747?îÿÈï·L@=Úþ£ßm¹À:µq5ÍÀ<~ùÛ"Ðå@ ¤ßðbÿ?ü2ÑɋϬ?È	¤"ZS?ÈBY@ãö@¡³CŽË	@?Ücï(
u¤ÇË?ïãՂS?ǒ£Ì´ú¿ÝiÀ8î¿Ýïø€¯½È¿æ«œ 1£¼AGNbllGB6 J0831+1746?ï»ê`ró?w'Û3Æôí?PÇ1Ÿ?IE¥æL~?~Aƃf¦ë?v8y/׺C?xžó?ˆµaµôåI?P¢Ø°m?]Þ¬uÉ?U?‡¾I×-?†‹q5íÉ?îa†gv?;b»z?qÅ>æÅà-?`1B+˜Þ?§®ñ²_â5?Œ>'?îØÇö7(Ì?"©²Sé5î?v¡Œˆ÷­?eø5¥nk@?Ÿ>žúè¨?ƒ~úŒYÂ4FGL J0831.8+0429?æzf©_èÑ@8YVŸIÀ8,vü¶ŸdÀ;«UãTÏ@yïJ%=&@rN¨Ú?-ÞM?³{1yŸ©(@ÃÉîËû@;ț9×½¿È••~Å¿ß4ä"ÔÁ8¿å$ŽTÁù¿ãŸLa¢—¿èþ5$¤û¿éáä¡ÂAGNbll3FGL J0831.9+0430PKS 0829+046?ïÇøo"·?s‰ººS?IA_~oGf?CÏ5@¸¤3?yV×Øg¼@?r DŠ÷¾w?ï%NÜ?•£Ïðdÿ?\Ԡ ÷Æ?{‡ß¶Ažû?Œ¤¢ *?UY8¬Í?ïoåw"–i?|WÈ~¤]à?lßlöoż?b9ÛÕÔýH?ŒÎÆá>t_?xîžÈŸ=˜?ïê}Q爾?Q˵V¦?B"äÝé?7'Û[ÓH?`Ý­?È?N3
€jÁã4FGL J0832.2+2753?ÚÆp8"…@@ ì•¿ðEÀ;8^B«v;À<¨PŸTÄ}@"Ô¿Šo@'™Ù;?П‹€Ò"w?¿_ë^C"d?ìv¥CÃ?ø3 Ä̊?ïñ`®–¿äë‰>ÿàK08¬ð¿å՟¿MˆI¿êg+R"!‹¿¶‡ä‰ŠÙAGNbcuOJ 250?ìJH">€_?³Hh'žÎc?4ІNò?wÒfͯc}?»‡#J;3.?²éŽˆRcq?íÃèGó™?¦ú±Û6@?Š`áˆG™?ëšG×?°EČ·€ï?¢ÖA(ˀ?ìÕBZœRX?›5T¯
4?'pnf"?AˆÙ?´¹Ñ©]˜?—`e^tÇ?êõ)ÁÍT>?'ŒHa6?Ÿ¢OÙÉL?Š'-pwí?ÀG¤®Ïuà?š•<Jã4FGL J0832.4+4912?ì݉èe@B1yЦv!À:A0«™v^À<˜Ç¤nß²@¾]r¡Þ@¾\ǁ3?µõÞ;¿ŠS‡;žÍ?ԘÂÚô?÷÷/™Ë˜š¿ßÞ¿þÞ÷¿ãc-ÌÁå¿æ®x?'æ¿ãU1Š¼‡¿å%yœÝò¿äF="†AGNbll3FGL J0832.6+4914OJ 448?îçå›ÇVÅ?–Îe´D?t¯8á< ?n0÷/¥*/?×~NÅÿ{?"Ë7"ÜÏ5?o]\?‡Æ¦îe?u=€M•­?1tëƒÕ?¡oŽ¯Wtˆ?™¯Ñ+< ?ík¾‹hº2?"ÒùЯaÝ?'³¢¹=?'‹dE:i?°^^ßр?Ù_!ž1L?îÝUŒÆm?'­¼òÌ1£? !}e'ÓÑ?‰Æ¹§®v?œZƒAŠÎ?"Åýá|;W4FGL J0833.4-0458¿ìÏÉVu®@4+"Ù@yÀ;çÌ,"ÝÀ<èj±NÂ@¦9$¹È¹?ú6çÚ+?Ôö+ÀÎð?åÞN4@ym@››]@'~ã	û?ﮔ"6`º?ְߛÜiù? +€À"À¿àvH¿ïÿ­?å`¿È~£®$kAGNfsrqPMN J0833-0454?ßüyq‰µ?Æ<
÷&]?ÛlèÛù'?Æé…Pdb›?²[úªSÖ?­r"Y뱯?à—áݺ«*?Ï}ÍAÂ7?Ղx·4é[?Ï!ÌNkÍD?›‡«€¡?´-«À'#?ÔZ*ë.ëa?´$E@àÞ¬?áˆB…ü˜r?µéF=Ó?Á* ¯Çx?¡õb:"zK?ç7PåO·?²UÃÔ:_è?Â%!|÷ƒ?°ÑëÇs9ˆ?Á—IFñ¢?£¬^Uk`4FGL J0833.9+4223¿ì»2Ôú©æ@B"ÂÎFIÀ9Û‡\€4À<uJïèZÈ@#S—+Ö@<A<
rJ?³ìhžyþ?¥z{TDP?ðœí¬@eK@
U€ºûi?ïþ,‹yEf¿âϕ¿ol¿ç'K³žÓ¿àmš7NJç¿í§VPn­]¿ïñÍ!ÜHÁAGNfsrq3FGL J0834.1+4223OJ 451?ïªI%ú.?€F–ˆŸˆs?ZÊ)Ȕv?SN
GÉÕw?'=4qHb?~"5<Ôè?ïNTp8šÕ?—¼ê­M¸ñ?hÂf"/"?ƒ;ì5҆y?"%6:q?'«Ù▂Ù?ï<Hò?'Èȇí—5?y{óg–Õ?uŠ³(?—yz$<7ß?}W»/±÷?îé?Îþí?‡Ót³Ðùk?"sM!b?'‡¡x®?ŒÈñ¦$y¼?tëÝÐ4Ê4FGL J0834.6+4402?é\?j'ß°@BFK†ýÀ:yÞfRDÀ<§—L¸?w@Ý(bŸ²b@CF uÁM?¿iS֖Ð?½§Žú¯34?üK‡mG+8@	E…a~J3?ﭓK¡¿¿s?|0–åy¿äO›HÆBo¿ãð`̞¿á²¬ÅÆHN¿ïü:]Éß³AGNbll3FGL J0834.7+4403B3 0831+442?ïÑl,eó?kÂYù[ Å?R3Å¢øš?LúCª£'?rãå¸dH¤?h€ú‡£iz?ÿ؃~?‡ª×0ƒôü?PøIp¹'¤?]RœÜ÷Æ?ˆ9vÛÇûM?…"ˆ²dƔ?ïXK†L?þŌq¹ä?pÁk
<
	?aY~Í£'¤?—ëú43^?|VÛÃ\Õb?ïX¨¸Bƒ?v.讜Š~?êBÅñ[=?h"58Oã?‰à°Œf'Í?p­öˆ8K%4FGL J0835.0+6243¿ìÁŘâ @AÙGNΚÀ:ê"@lÚÀ<ˆ$GÝå#@SÒ¾SbS@<=3g6?øŠØ¡e?¬À'¤)añ?Ø9ºáè¾?úu…•Ö–z?ïþÛ½«q³¿èÝ¡ÜF¿ífÒ1›Ä¿êŸ—£ö¿ïJ˜ñÓí¿ÞÃÓߐžÉAGNbcuGB6 J0834+6249?ï'2H\?²ðxfý»I?"/ÂÌa?²¶IªÓ+?…xP×ë?‰gÀÉÙ?ìµ9‡Ÿš£?Á¸}8ž?¢Ò	˜$?¶ÞþPÈê:?°í/=wÞÜ?°u­Ýæü ?ì/Ž³"¥? 'g'{ª?—òVùËg?Ž€íP$?¹1íËñõ?œ*räÂ?ï/•a¬Wã?¤~¶wHÌ¢?cDBû£ûÎ?"iŠV'Yÿ?—¤Ëk" ?¡¨±pvJü4FGL J0835.2-2243?íå_â¤â@%›™N?À;>ŒjÜí¬À<߄ۜsi@@'I}"@	ۛœ©?Ö £ylS?ïÿülò@ÿ3å	Út?ÿ4]q +?ïñô¿Zƒ¿á½Zi¿àøú'0?¿íÔ-ê¿ïîÌț¿ííËJÍÈAGNfsrqPMN J0834-2241	?â{οÿ€?ʂվxL?Îm2#ÙÊD?Æ3¾‰‹?ÉDÞ¡&7»?Œ3ÏG¬Ç?Âá|÷µ.?ź$ªŒ?ã¸P8A?ÑÿDèðR?ÐaÐãµ^q?ÇãQ±éC±?Ý (ãë?±"»hˆd?Ñ®M7oNà?°¥Äž+Qa?б‰å"'3?¨––ž{<\?±uÕºÌæ?žÊFY¤ý?뇨ï®#J?­é¼³!?²LâȆÍ?¤†ìbeŽ4FGL J0835.7+0936¿é T5ƒ¼Û@;"È6eÛÀ:ÛÉÃ-ÚÀ<Š€Þ·°Ü@Êõ7O!¦@·{¿"ÿ&?ȂÛgj?¦"¶]Ÿ˜?ã—ñ=Å]m@ ÄÃéÏ<?ïûB0&8¿Á%l5³@4¿ç¾"7Z	¿ß@\[˂˿ål¯UÀô¿àÍÛÀ…—AGNbll3FGL J0835.4+0930GB6 J0835+0936?ï=U%S,?‹þjRÉ5Ã?Vý5f0éÐ?G«	0¶ï?–ìÂò‹¤?‹|ÔéAØÊ?ï€qp-à\?†íô?H6ºñI?T¶œG:?Ž`8Ev?…ÿñ9ç}?î•K¡ÑXý?‰;õqÌ?s Cµ?b¶þq9VV?¤Iƒ¡ÖgÁ?‡ç;(?îÑÖ˒ôË?éi³Ý@°?wæÎ¥6?^­éE¦ùÑ?ŸËs	xÙ?~‹Ž/Kf¨4FGL J0836.2+2141¿âåà1X'"@@'óUÎÀ:+?› 'À<b¶FxŠU@ìõ[â(ÿ@ö+ —ºœ?¹|ZÞr習"¼\‰/?Ôg˜*-Ðô@	õ½©Ä4"?¿É읢'½¿æ©ÛÑLŽN¿ébÇ«$ÜX¿å<÷‡¿ïtRQÜl¿íoÙ¬¯ AGNbcu3FGL J0836.3+2143MG2 J083615+2138?ïÄhT¿ç?'¸ÙNÏS?l#^Ò(	?Ûá>g?otLmðä?…xþÀ"?ñð#Õ?‹Á'¤†¸\?Qq¬%ÇÎ?dm"::}?‰®Mÿ>ö?‰7JrÉ/?ï-
®ðeú?ê"z‡p?põ¥€Þî?Z2¾¾y.W?–7,¸"è?|¤.ìGý¦?ÐI ?qo‹øÍ#+?v³éŸÉºy?d™ÊV¹Q?€xI|º'?fIo6¼
w4FGL J0836.5-2026?ËyÖ꡸¼@(9	(­ûÀ9ÞØ-SbÀ<&æ"Gp@rxJ"xÈ@¢|—*T?Ã([!?Ò7ö{ò¿¦@)È»ÆL@	ÒÀº컿ÝÑK·Žw¿ãŒk'fL¿ìæMÂ*²[¿ïÞï@4£¿ð?ïÿþBe«+AGNfsrq3FGL J0836.5-2020PKS 0834-20?ïʂ}h‹*?m|ˆ–ÖŸ?axüOL]é?dº1 3á?rC$<í?xØÕ£š,?ìã,—¤»€?ÀujÑÔX? %39—ìo?±ª3XL5÷?°Ô¦-»?¶"–pU&?êë7cÞ¥´?¥›¹7ö&?«ÃxõËóñ?˜!E'Zî¯?ºÄˆf$Øe?œÁ°ùš^i?ïÃБ†?‡øXìÎ{?"|žÃë?rHJ?"ë‰vmH?'ýgÙ²á4FGL J0836.9+5833?à_Ú8α@BDaAcwŸÀ:ÆWꢠ©À<¦­@?‹0@¡¸Ðìl$@º:Þù;?¸a.n'z³íPÑ?ñ–¿Ê…Ë?ýq
×tp•¿ÜÏ|¿ïÒ¿áN
>¬ãù¿çh?ŸR@?¿âj4¼ .ß¿ã"2þ¿Ø­JÜKAGNbllNVSS J083705+583151?îûÎRá2‰?Žeþ|—Žö?y󶲏ä'?kà£Nћð?š	G÷5µÐ?‹–°,<ëD?î¾Dí¡¨??›?#Æu?lT¸p."?uî<ÚÃc¡?¢Ve¤^y>?˜zµZž?íïXHÎÒ£?…ՏÄD?ƒ¤Ëv@?r@Þ#Ýò?¬!y@Mx3?Œ¥V‹Ãǒ?í³,¨Ëþ?0+}‰Àk?"ð·Ì¨­?\¢è_è;?ªVٌëÆ?S–"yš4FGL J0837.3+1458¿ï"Y¥¢@>ȼœÓáÀ;)(Fp&ÚÀ<§p¶K@ ö
³\Z?ú'¢ê{3}?ÖÒ"4ÕË?Áéoo¦V?ñ¢.x¹OB?ý1D‹u>›¿ï±E½yr³?ï;ˆÂ0ç~¿éT•]õ©?5n&NHbo¿ÞëF'¿àª|uœdOAGNbllRGB J0837+149?ç׌p?7ƒ ô?IüæŽØf‡?D¡¢™åÅ?‡¹÷¡/]¹?~"÷.&n\?ï]ü>•?wãÞmc?S'"+ÇeË?bgÔ¤G°¡?"Oùƒv÷?ŽlæÇÔ\?íúŠX´?ÖêäFÛ\?v`"AF?eÀ¾Iî´?­‹V,–+÷?ŸB4j=?í–[¥$Ґ?•ë…àÁ?v:k˜ês?q92`¨ê?±ë0Üà?•.såØÝ4FGL J0839.4+1803?îõZ»ê@?¶·ª%ÙÀ:`þU/ÝÀ<€VAU5@ùZ<a…@Ž±=û
R?¶Ðó-‰¦¿œ܃yË?å±
õ´M@»<.Y"¬¿ËßÀ‹t¿ÞZ~¦¤¿ä	`0Â?«¿åJŸb0w¿á•`Nõ1¿ÌBEÈa-AGNbll3FGL J0839.6+1803TXS 0836+182?ïº	8N¬?pýNy"ï?Røñ)uÅU?I¦m«˜Ò?~=<{8<?o-酑©R?ï³QºoA?*†â/?@>ÔBÈ 2?P_"çl?':~M7­º?€êîëß«?îÿ'ë E™?'÷Ô2C@³?n%?"'?ZÇ´W¼~s?œZôºG?U'š6ÚÁ?IÓÈæ?oTݝkJo?aD{kGwÔ?L'†3sø?‡ÎN°;è\?nGç³ØÉ4FGL J0839.7+3540?ÄKÛÃ>f@BA,üœÀ:RÆvqvÀ<ozLÍ8-@ãÿ:³/B?þ¬€&+
?ºÛâ~å¹-?¶$[T ?ü§‡H^=£@çV:õ?ïþ7+æ8¿â¨Oªb>¹¿ÙÀ[¥B¿ÝP»>Z¿álšÈmÂ{¿â	P
ÚN–AGNbll3FGL J0839.6+3538NVSS J083943+354001?ïde'½•×?…¼œoQIÖ?g¾^•uÝ?{%ZÃTa?Üz–?~C4©Ä£?ïøÛ®¶u?'uÏR#ƒ¶?fIÚµÊÍo?oß*
€s?™—©3o×Ê??¯0''?íµŸå@µƒ?"!Ó(ïQ?'ÑÞô¦Aé?rSy"c?¯ñ‰îËV?×ÿž­Ù?íh?
}Z?Œ8˟S"?""V-º?wÛLoÖ&?¯9äžb#?‡ Ù§—
4FGL J0839.8+0105?ÙphJ
·›@8uà'Œ6ÛÀ9™'ÿùJÀ<Êþì@æAzɟÇ@î][$éÄ?µŽOŸ¶¥T?ȟ©érõÁ@ÂÇut÷#@~‹ž":¿ÓÐÂÛ\\¢¿à"0±x³p¿äSø:8àò¿æýNª‡þg¿ïþôx
¿ášXÜ:(AGNfsrq3FGL J0839.5+0102PKS 0837+012?îÛ*:d? ÎƝ¸W8?˜¿-±0n?˜M†{¬À?‡¶_–FH?ŠX)UÅ(?ïyzþÓfW?ŠÂס%c·?Zß&/n?j‹<O}
?ŽE[…C¼½?‡æ)èû3Œ?ìzÞdêø?¤éOÇe‹©?ª´œr-¬?›Ú_Lz?­ž!ï"Ö?›<ƒ À?ïuÉíg"?s/ÎUï?rEŠ^ƒ?^•NÁåP?‰j¿´öÙL?okãÝل¿4FGL J0840.8+1317?ç¾:"¥¡@>10ߛÜjÀ:"ÒÊ<ϔÀ<s¿T>E¶@¼è7"î@ᶃµ+Æ?ǜvXKñp?е£»[‹A@9E'Á@ÚEÚ)ו?Å?ïÚê¿áGïþU0¿èŒoz^Ù¿ä0|ŸÏ¿ð¿ïù^Æ^ô'AGNssrq3FGL J0840.8+13153C 207?ï©­Pš€?…()ÈZ'c?qñÎÎu*+?|´J\»?y7‰)½•Ë?y
aŸ_h›?ºÄA?Š1R¼íˆQ?ND.!p:<?aÌ«soD?ˆ¸Nlؕ,?‡néÇe?í«ù¤Tðž?—;¯<Ùm¼?•£;^bB-?ˆghó^'?ªnÈÕ
?ïS½Ï¤p?ïÔž*¡¥?q$åkp£?lÃð#ÀW?VqO?#¤Î?…YÜlgX?mRfÆI™4FGL J0841.3-3554?çˆè>ö¾k@
î¦]¨À9ÃOu‰À;š$ˑc@ X¢õãÇe?øáS½vd?´kë
¥u?Ê:
Âá@d¼~ ïÏ@áé{Vw¿îHPÑ©«?ș5[+ŸÁ¿Ì}†éh¹Ó¿ÆÀUÛ~ÁQ¿Þâ›ìK¿çÏ,ù]OAGNbll3FGL J0841.3-3554NVSS J084121-355506?îÖT½ã©í?˜YûœÏ?†cã¶<®?…¹'ôú?švhlÁÆ?"•J¥wx?èv&Fȍ?Ƌ"lðê?ƒæÒ±Œš?šô+3^ÐÇ?Ìèù¹ÆÀ+?ÆV+p5aÛ?é`8·ãëí?°Zþ,4?¸ó89>]?¦¥÷]ÿ=?¼öG§b??¢êXÑ»Æ?êµ³Éc?§Ež¯'ÿÝ?öïÞOÛ?}­Ðò}à?Ŝã-f÷—?§:æøòŠ¢4FGL J0841.3+7053?â??dm	@A6T´:çÀ7ÃÜ«g!wÀ;ÁˆÛt´@±'!PÔ@2R¯')?"r×
•ž?͛¿«Q'@,2'1ìV@ Aa*½Bì¿Ô'Õ…-%þ¿å¦BWéK¿ëƇÙ}µ8¿íTÞ긿íäÓôß:Ž¿ïï ×{|xAGNFSRQ3FGL J0841.4+70534C +71.07?åü3\I¬?ÊÍ̃@Ü?Ó¾>5<N9?ʵ>;kA>?rVČ_›ú?|?2ËSR?ëRùޖ…?ÉóX m?´GÄj "?Âpΐgü?³£Æë-³?ºu'£YÒ?æís´}‰?´Ã¸½?Ǔx'»?°Ñï&v¿?¹mvX?©»ºÕü©Ö?핰…L£d?¬¹¨u
åý?¯'8'ëSà?©–üæy¬‡?ŒŠüe)×­?Ž%ƒæш'4FGL J0842.3-6053?í1_ÎÇ£ÃÀ&µÅäêÑÀ9P—2·qÀ<§z¡‡@*#ô&@ºÚâ9Eœ?±j=¶nçi?¸HçÐ^QÅ@1düÙÚÒ@U"–Ó?ïm­íät‰¿à/Z`ž¦I¿åt"狕¿â"ӟNå@¿åbUË
¯ì¿ïÿÑÜ×AGNbcu3FGL J0842.0-6055PMN J0842-6053?ï¸Zuã?".h8?FÿPJÛÛð?F8L•ÇC?€‹Ç$´É·?ƒ'¬
Ü4?ï/%:[Û?¢ ra5¶?G^ŽYqËn?gjžîJ~l?™c¦åèö?¡¢mì âÎ?î¾ô¶=!??Œõ<MTB?t$vKðÖ\?hiÓ¯wÒm?¡Œ%Ò¯ÑE?Škên*"?ïc‡6j.?wµg)/e?tŒæ2Jd?`//³ð	?Œ×¿e@B¤?tG=þݗo4FGL J0842.5+0251¿éóú3ô_t@9é™þCg^À;$r[UÀ<©F<û3@ @Öí7%†?þJÅ 0!?Ó͝aûÁ?¹%OšÇìé?á8À ý@VJyö¼
?ï')}§ËŒ¿ïH_	B?Þs[Ao6¿ßf'd@ò9¿ââÒÞßM¿Òä\Xp"AGNbll1FGL J0842.2+0251NVSS J084225+025251?ï);ç"?8ä®4?E°9
å?;΍ÁÆCƒ?š+:Ïn?ÍDM'?ïül³<?œº?Æêäm?e¶ž¹•ð?våIÍ?œ‰ž'iš?™™#Ù¹@U?í±Vy£I?•ùõA–?q±Á)	«?\6¸äA®?±[qÓ#f?• D)sÌ2?îer Yà?Ž¿ùó6ç?\æÿv>es?SÝ¡@
@¦?¨Á¥þ½ŽÓ?Že=q¤4FGL J0842.7+6656¿ì>úz–/h@AÎa(9.À;]u&ÊÀ<›ÚGÓ
@!®â‹ÐÙ!?ÿ`›KJ.?¼_ÿ™þ™N¿¯ž
œ µ?ðçáuÑ@\.Ìò¡¿â%NÂR ¿è8BÒ§®¿Å›
bE'¿æ½™Þ¸Ý'¿Ð'xB±ÖQ?ŒâèÂAGNbllTXS 0838+671?ï	yd0Yê?™þ1Æ)$?_Qª©1˜?RÍîkâ?œÛ¸Ïa±{?™ª9~`d²?îÓ;¤J'.? ÷ˆ®þ£?iäŠø9~Á?yhဥó½?¡-ýÓE%?žOʄ²äß?íÝ+ð?oÆ?'$î"|?tÑ8*% ˆ?cìÐqî^Z?¯"öÄO?_H×÷6¡?ìw¿ùD0?¦ÔeeB·?s$ƒÃ'_?o°°'-X@?¾J‡ù¦U?§6½ª%‡4FGL J0843.0-0853¿ã[€Ñ™@3ó)¡¹ù‹À:æž&Ç&À<ƒZ­ËÆ@0]^*Ü@^/æw˜¾?Ò'Y
]Q?ßëSàý±F@p¬bÉù´@	Jod綿Î<x{í?ßÅí οæµùìÀˆ¿ëÇ(}͋9¿£ CX´¿ïýè˜Û-¹AGNbcuPMN J0843-0848?F=×ù?£1vvãô?"f¥ÔtH‡?™ûB¨eѐ?˜#'cиP?"²ý¥–o¤?_z[ˆ?­.Þð8e?…U ¥ƒA?™t¢š?¢r"À0æ¥?¤p«àèÝ?쯘áôÞT?®¼€ *?¢>"²	pq?'¨wÚ¿ž?±cî—TU#?"忘"Mé?ï	à0ì?†'-¸|ÈÚ?t«Uãõð?n†¦tN?™™$sNÆf?ƒsMXGT4FGL J0844.2+5312¿½[ÚeØ@C÷…À9v}¾qÀ7À<QU>S"@×Àvþ?ÿðU2a|?ªß™ƒX?£¬Ð6f?ö²³"&k@NFæ™Q ?ï®Ê榓¿ßM™æÆs¿ãN4 C€¿Ö ËQ¢Š¿ä¹ø´²#Ô¿é6ÈééAGNbll3FGL J0843.9+5311NVSS J084411+531250?ïÔh6'¿É?'D¿ö&??I¹ÀG8?P>)Èqí?s×I"›§æ?€eXê%Š?不-<Ll?"5qÞ×J?G]"CçÇ1?Xü?oWJy?… \l®há?'yTD	Ðe?ï<GªX…?|]=2?f¡Øu…?SÜ´¦B5¼?•¢è¢ÆOx?zVa'Ú19?磊Êoi,?kFÏP°ÑÆ?l̅•Ÿ6?Vb	ڎºí?~Õ×ýÈQ?e¯u·'©4FGL J0844.9-5458¿á+€({ÁÀÿ«–òmÀ8Û}½›¢À;›ñþµ}%@|"©¶Æ@7G"ê?©b}=µÌ?¸?ëÓME@§,å;Xœ@¼ÓüìÐ"?èJB1}ѿڅ]à0¿áT¬?8¥
¿Þ_œ}y¨c¿äñÿ¦™¿é̪ÍÛÁAGNbll3FGL J0845.1-5458PMN J0845-5458?âÜÿôÐD?ÁI'!Õ?‡'Éx©qr?€ŽÂÑ-1?َ¡´Që?Á/-cÄ#?➏²-?Ì%úàðœ7?¡aŒÒ—Ñ0?«Ÿ2ä¾?ؖ°C‰¡€?Ë=xÜÀ¥ü?é¸\JM¥?­'¹Ý5Ô®?›èPoJ(I?ŠØ¨'nME?Å¡…Ðí"c?©¹éSÅ8…?始¦üÿ«?¥êÚ§þE+?±t7͵¿6?ø2Ô	¨?ÐSÚ¾˜Ü?¥`?ØÞf_4FGL J0845.4+0442¿æ>{ÄO-@;lÁ"tŸÀ;OsۙïÀ<§7T*@NI.B^?ÿj`':O‡?Ϫ÷¥h"Ï?ÌûÊ;M?üÿ¦sœ¯Ï@¿P¸TE¿ïÿVø4Y¤?ïõ–àVÂZ¿áúØC""¿ßIMì¿æ¨ëÎE¿ïýøScTcAGNbcuMG1 J084516+0439?ﺮ϶?uŠ³üŸ¤?\Gù76?T
!'Ȭú?{è¹*J]j?r¡PA¸©Ç?ïa<þ"Ö'?ŽÂpJK?[Ž"'£H?h²«¤'—?'võ:ûX?Šß"¿…"Î?îRY¸«
_?Œ
Š(ðÕW?~[ù܆?nž=\îlC?§å9ËéB?ˆ)"¤t?î5õÂ?¯&?Š}Zg?"ÜÔÔªÃ?on›¸º¸a?§},¦Ïâê?ˆÍPÓùÅÉ4FGL J0845.7-5556¿ïœqº¤ÎxÀ !¼jfÀ:‡;©À<#ú±¦@N§¯ÜÑþ@OIc÷ ]?·hã²°¿†–]¶$ÐÖ?Ï$ô×è?èE`üçi(?ïö€[¯ÿ¿à[7¹ª±¿æ÷a€£~u¿ãtUªV€¿ã}éµí¸¿ÕÁ›ì/>AGNfsrqPMN J0845-5555?åhKeñ?Ä&åm&>?Žvˆ!°?'띋1œ?Ô>Øý€£?Ãàn"[ÂÅ?Òtñ¹ƒÂ/?ËjãĐ{S?•€3S9? dö°î%5?æ'9¥LP?ˇ nIp?ç<1ª¾?© á»[ ? <´hÄ?…KÈj;<?ϤW:Ö?§$
<øBí?Ûï›î8t??°¥¥¸
£?Â@ŸD'?§ç–›aŒ?Úðo¼ˆ€?°pr>ðÇ4FGL J0846.5-2609?'ê•K€Ö@%(:û~'À:ž>Ü´¡]À<)›ûs©@"	ªÎ @jÀÒÄ?ыì\ßÿÚ?Þ&S0/@K}\L11@Àíñ_©?¡©³m¿Ù™·@ôfð¿âm5Þ^s¿ë?nu(¡	¿ïÿöût€?ì.¾ù¥sAGNbcuTXS 0844-259?è=CnEÉ¥?¿W^;è?Á²÷ó?¶­:…(Í?º±Öž¯ÌÉ?³–i[ÆÈ?àS?Êþl?Îǘ—ýé?ËN³%ºôÅ?ÆeÇë|ù?Ѳ&×&€Ä?ȉÔ
§?âíµ<¹¾?°Ù˜gï•a?ÄPœ0þ?£pëÝ[?ІO8t?©€Xb9³?ÚΑ'¼Ÿ?°Q¬Ê‹Yu?Ò,C½?´¿å5,?ÓÑ+¦]?µ|:	]E4FGL J0846.9+4608¿ÒÊ®aI=ƒ@Ce]€ä–îÀ:Ò}qDçÀ<–¦¾EJ@	8NÐóx@Ü{£åLö?ЩoÐrt?Á–ÌR֒?ë¹óêH@qð]J´¿Ö,DA"Š¿â݀y7$¿èÌOÏK,N¿éàkB"#¿ïÿÛ¢¨‹û?ÈXp™ñaAGNfsrqWISE J084734.29+460928.0?ïÁ÷½$Ÿš?tØ=ހïŒ?T)­Ææ¹?Os'Îãä]?yù¶(~y[?s…ýtñäj?îîsEPà+?¶4'@)?gÏæ€Æ)?vEsŽ…?Ÿ7š…Ë70?š¶$r1B?îÝˉKƒ?5iÞh?~¯-O^‰0?k™ÇÖñ6?ª\=v»?Œ!ÑDüx?ïr–€ýR ?v\ٍŒq?oSrµ•Ê£?\gäȹ?‹…ƒEåË?sz°'"&4FGL J0847.0-2336¿íSu̜ @(hïܜM©À9×u;À;Þv˜Ñ @©lut ?ÿ
ÈÅ×F?§øä?'›Ú¶š?ì[?pé!@ƒÃŽ?ïÔv_î¿ÓŠ¬–Ì_À¿áGOµIùH¿Ý¹IbI¡4¿ÙËÿ€>T¿âØÄL0ZAGNbcu3FGL J0846.9-2336PMN J0847-2337?ís;4G??¬Aj¯ëH¡?fBÍk7œ?`B‹ëf=?³´óÚlM?«Û†d}êç?îÆä>éŠó?¦:÷º]b?a3å™Ñ)?pš!»ÄxS?¢~}·Ê@f?¥ªSôO?ì4}éމº?¢‹ŒÖG?‹F?öxPö?|m»ë?ºóH²<¨? ì,åق??ìçnõ¨ñs?™U ª+X?'/¿[Y‹?y¡©.:?´x˜{â0?–­xñY£\4FGL J0847.2+1134¿Ð%Pʦ_ƒ@>æãK"SÀ9꣩½ÔÀ<#¥©rU@ þy{Añ?û4<G®ë?´Å"Z‰?£"ö>,­Õ?ò7g«
f@ÀÞöÅð¿ï½µ¢ä›ö?ïþi'jÑ/¿×JC˜e¿Ü¯ÎD¬¿ÝXÏå[?ŸÐňhwkAGNbll3FGL J0847.1+1134RX J0847.1+1133?ïÔ¥²Gô?hª]´N"?EŽtîÁö…?>=#e;"?rû­	Ç?f)X.ñ©z?離Èý­?…Lû§9}?Gî߅ñ…?VF–û¼Ô?"£nÒÃuÄ?ƒ°´N­ë?î´yÆò‰~?ˆ¹6 >X?nò™!"tØ?bÁ  ¢I?¢É9þ¿ Ì?††	ˤR?îW9‡éFƒ?†²°ÀœÉ?xC«©‹?bͧ|åŒÛ?§"=¶"¤?…Ü|Ni4FGL J0847.9-0702?Ó\Áع%a@5ø`»+º™À:xºüÀ°À<dÂI¼´@úc"9:ß@°;#Â|è?¶ù¥rë¯ç? @½+ç\?çÏAò×s@ÁÔÜ:Óæ?Í>^!"¿×¦Gݏ<ɿ凾s˜©¿áè<à8Ï¿ä ©¡Nš¿âÎ÷IxAGNbll3FGL J0846.7-0651TXS 0845-068?í±Ãq7½Ï?¢ç°nÑÕ?
B­?reҗuãœ?°P<5¬n¦?¢	–Ê´?ï
Ê0:¤?‰¿idöi?UÝ¯?dO!œ`6¦?ŠìÏõ³}?†¾YŒæx"?혿F
*?œ½—wÑ#?úeDÉ¢—?€KÆŽƒØ?³Œ ´.?˜³àæóÒ¿?îÚô…PNÛ?}ã'ÿ-?‡Ž!ùBŒ?hÙ6mÚÉr?™¨Dùƒh?wÐÊïµy4FGL J0848.0-0524?ïG>à1ü@6ÛíúCþ]À:À›f"À<cþë-
$@5?Ìt@3i3 @}?ƀB¸â4?¿v
xc"ù?ô¢ŸÒ˜¾¨@Ô
UÓò?ï-©¼&Œ\¿é¥Œ#Wô¿æOÿAi+é¿ï*Ú~çÆ¿ï¡3Œ†Ô¿åT/aíZâAGNfsrqPKS 0845-051?ïnj½Å±?}z
o&á?^OÉãh¬?_#'áåtZ?t¥®¤šü»?z2.n¹F?î`£b²B?¢ï¢ŒBO­?ƒrRKͬ?Œ0Wf¡ÐÈ?¥5K1pÓ?žç‰óéÿ?íPN|aC?–%¸þ'Û?Š–ÉñN•?xÝ,AÍ?²*¶%ó#M?"ÇÊë\a?îSôý÷‹?(Ú

¨?˜Ò-o1Ú?…bݳú­—?œ¯2Ñíeå?'AòØ"º|4FGL J0848.7+0508¿æy
Éî²@<Zþ`Ï6À;U$H¸À<xæÞÆÊT@"øàå³x"?ù·Ab ß?ÙC«QÎ?Á"¼:-x^?ð:CȬ¬œ@ߢ8y™¿ã^V݇Z'?ïƒ}ÎaøC¿èåÛ&+ã´¿á:À›;/¿Ë¡£é©§Y?ÉqŸÕrã¢AGNbll1FGL J0848.6+0504SDSS J084839.66+050617.8?î4W3‹ÅÀ?¨æóLÇe?Yósxìb©?YºîÍ
µb?«êñ+|@Ù?¨eQ§fŸ?îa‰ª¸H-?°,ˆù?rùéÂ+Õ?ˆ{$ÁªÒª?§ˆ(6•?®_t¥Sg?í†JÛ©ä?—þšª‡?rzCÏt?c–Õ°ù|?²¥±~zٕ?–qԛ¯?é›~Œõö@?³ž3Y?"R?m³Ù•VØN?pù		"¯?É6eÒË£?³çl8Þ,è4FGL J0848.7+7017?ìg—á*@A—Ô{í·(À:£`ó_ލÀ<½ùŸ"®ž@ 
ÜkÒ6?ýDãü";?ŞÜÏyOw?ÍvBýU«®@ÄÛÄ·T–?ÿȃßÈýà?•¬g@o˄¿æŒKgÝ^ë¿Ø'(üùe\¿×m›¤`Çì¿âƁY0ô¿ïÿxPsµÚAGNbll3FGL J0848.5+7018GB6 J0848+7017?ïÕ0‹¤â?'™A›¥Ž´?‰q'('Yµ?…RÊø¼Ó?ÚB¶Ë?ƒ§lÁ¥?íÔÑÆÍÕç?¦ù-Õºv"?A	`3%(?"·a'GK?ªâ¡;Ø*? "€íqfq?íPk¡$þ'?™+/þ?'3hb¹,?‡`­hPú?°ØÖ¿]¥?'8äîgÐ?ë=ía§?žB¼'…?ª^þN.?'ùžL«?¸ämàœ8?™h™3U4FGL J0848.9+0205?äMˆr9@:îU7«À;(&x9́À<'IÅEïÎ@sñÀ¢@"ę?ÔÀü§…ë?Ån"›þ£´?ó?ª¥Z—ü?íqlŠ†·?ïøgºú<r?Պt";¿¿åüfîK¢–¿àÇ&/>±ì¿ïè5sS¿çåÇ°å;AGNbllPMN J0849+0206?î^f³{¢?¤§<ÈÖ?ˆóîìsr±?ŽÊGKŸ?£Ü™[i=?¡ÚI	WT?éwÒÍXô?Ã^eP›Ç?·b¤0óÉ?¾0¦Šs
?¼ÞÅdško?±ÀŒàž!?ëÔ¾ëI'û? y;ˆ'??Ÿv"³ƒ]'?Œk.!S*?¹|øҘÄ?›Tø…ŠÊ?å"5l,?±œ?ë1?ÄkðâÌ/ò?²ï÷N—?Ç9ƒ—^?¦"x*·4FGL J0849.1+6607¿Òэ{ÔÛ@B7•=êFZÀ9î.C	jÀ<}Œ†‹ŸÜ@qd<ëmÍ?þӀ*\ÊÜ?³7çßï?£Ê© ¼'\?ñpÄÃéÏ<@	B6n&#U?ïýå^0´¿ß¿ziR©ñ¿â"~§¥Ì¿×™ÒduÄ¿á‡.'ŸW¿Ý×åÐDAGNbll3FGL J0849.1+6607GB6 J0848+6605?ïÙ`©¶a?kf°õB›é?G8»V€p?`]ÆÇ??ph"¹ÿfÈ?c¡
ƒ‹O?ñŽ_?"‡cÅE˜u?Fÿ+øV€?S
+ðƈŸ?†¥Ï¢ù?ƒ1#¶XZ?ï(¶>ˆë?~Äò{çÚ?eireŠT1?Xí/[x¤G?˜<	ò=˜?|b¹wHuà?ï,³½Æþ?ygrºKbô?{ú'.+…#?`fŽLÏô?"jù¼¼??v&=ÑÍ4FGL J0849.4-2911?ÓX(+ö²@"nf¼˜¢À:¼i¨:FÀ<=MéDÓ@Ï`¾1@heD'w?»@DÔn?³ëÉ(]±?ú
üÈ=@|U\'ô?ïþ!8^ì¿åt ñ|¯~¿ß¢ûB+¿ÞžÔw
þ¿àG†Â&€¿ëˆô›GïƒAGNbcu3FGL J0849.5-2912NVSS J084922-291149?ï–šè?·Gu¶?I¯H3vÁû?DÚý±‰f'?›ß²}GJ
?ŒxŸñ[p?쬎Qd¤À?¼"?èí «?S5""Çö?f)ì»ó:?ºN·"ŠºØ?¼Qµ¿´»û?íax§5‰e?–ÝÍô»zÅ?xÁUöb	-?i%NŒÕ(÷?³h%fí"O?•Ï^·n_¡?ï	¤	ýþh?xˆº¦Ü@€?j6½Ž>?Qέøöóå?›"»èŸ¡(?w•iæ	4FGL J0849.5+0456¿ì5ùø0K@<pÊ>}QÀ9×KÞ$ãåÀ<#)è0Öb@‹v9@îš|îh?¸æg¨…ŧ?¼ªŠ,¿%Å@ዻŠ…*@ÜÁ]Wõ?î™dÀsøö¿ßÈy`¿'¿ß"C")m¿ÙDÜޒȿéA¢a¿7¹¿Ûlk"¸¼ AGNbll3FGL J0849.3+0458TXS 0846+051?íÒ{>@h?¦Ä|s»,Å?šç̕ds»?'¬éSeSb?°§y´ßÙ?¢ÓnQ'ó?íç5]hO?¯ÅŒš?™…æ†
è?›ü?r?çñ?±L³zÊ?¦›8RÖÒi?ìŠë¦D0? óØd…ƒ?™5"ÂL z?Ž>F¸ædm?µbŸò:Öb?™Õe¼97?èTÃ-¿M?Ÿüó áx?²oªÝWß?šg¯?ÆjפZVÜ?›5ÉF¼B·4FGL J0849.8-3541?ï¢Úú¦¾Š@ßãß8	\À9"8½¶¯TÀ;ºƒDÃ~o@X®ýÙà@eø5/?·;F}ù}?ĺ…aÿ#Œ@	ÂJ'k~Ô@Ž–±1ç?é¯,ÅÇ¿á–kðL¿àÈÔ_"8¿åþ†]§¥÷¿ë]Ñ6¾Øî¿Ì[ª
U‹AGNbcu3FGL J0849.9-3540PMN J0849-3541?îøðiD…{?"ÆUR?r,ŠÈÜ¥u?qf·-ݪ?œVÐ%8'R?'YÈΕzS?î^
«?°œ"…Ë?Pyßlî}"?gBݷѳ?®–Os½Ûó?¯ùq·¬›è?ìC»bãúÜ?¡è jE—?¡U#¶çÉF?'Ù-˜¡\?µ7"
lDy?—dÀñ=u?îÚôvpˆü?"H ,àý€?jsSÝC?Þ?VV"ÈÖD? ©ƒ[#<O?ƒJ\Åø4FGL J0850.0+4855?åØ^Z ¬Ö@C¢õ#-+²À8¬ß½jY:À;åùɅ°@ðI°ù½@Ê]†ÃÔ?¢E!Œ¡?«}~o`z@¤ûÍkX@?X@]é?³­L¿KYñ¿ß^y½±%ý¿ãI_à:gÛ¿ãú*~å8¿å±öQo^¿å8!WnAGNbll3FGL J0850.0+4855GB6 J0850+4855?ïÀô&ÌûÞ?€@e.2?BfçJ?<Ùc…T܅?}D‹¥'Œ?Ž&'EA?ïŒ\ÏÒ¾?‰Öuï3P?Nõ S
Q¹?a´ù_äâ?Šùz£T?ˆˆKÍy©o?ïIžÅW?†…Œ:À•?s¬Íñ#r?kùƒÓ²ü?˜‹˜«@?ƒûŽÇ)Y?ïôK¨`j‡?CÙru-?/ĔlÆ­?!9+®üe?Sp±šºÀ?Aw¢Í+"4FGL J0850.0+5108¿Üþ‡µ	¯@C'û îÙÀ8¼$>úèÀ;üyx'â@æzšÆë@IzŘûå?¢ïÁÄ[D?µC;&x@¸ÁƒÃn@§,_›–¿Üo1CD¿Ý<+)yv¿ä0usI¤¿äûR@ê€è¿æ†é"¬ðŽ¿æðc?jyAGNNLSY13FGL J0849.9+5108SBS 0846+513?ïµø€Áb?zãÑ8‡Gu?KNj•?A«jm—õ\?€ÑcW	ö<?yé.¸Œ–?ïBÜm"?»0‰Þ?H…ÀTAL?ZÊPHð‡?Šfðè³ó¸?ŽëMÁžú³?ïÇ
­S?†T´÷"5O?uû[¾èo9?pbCЮ÷?—¨FNð9À?ƒ0@¨ä!~?ïû®¯
Ħ?1c-`xà°?¹l©G–?*ŠíœÒ??Z±ÕÊ?0K÷54Ë»4FGL J0850.1-1212?ïË_r^õ·@3‡U¼Ê÷
À8w1ÅÀ;Ê+"Ù@y@¹åCç
'@<†™Õ?£3ìk£'?¶tJՑA†@pO'RÑ@ßSŽê"¿ÓW‰ÿ¯~¿àæ¯â[Te¿ã‰»€Hj¿åãZb¢®¿éêk
•ù¿äna|òšAGNfsrq3FGL J0850.2-1214PMN J0850-1213?ïÊCt|$l?…t'ž®¶2?RŸÀ~ö_‰?PÓS#Cöï?v6U¢01Â?"ïЗ?ï³lÉ7?ƒ‰Ñ¶J?JM2ö?_¦Ú%à?–ïú˜¡5?ÿl\³Ú?îóx÷Q–4?Ž±ê‡ô&?ƒ+õ
¯«Ú?VCsJ>?—úæŽõc?‡CÏuÁ&?ïõõ‰:˜Ž?D'Õµ
²â?%ØdàðÜY?EΗ•ý[?QYàî°Æ?BßÒ´<½á4FGL J0850.5+3455?ïúk²fÖ4@CHå£]gºÀ:RLƂ/ñÀ<‰I÷šÖ°@ê3ß*b@M~ˆœT?¶ç\20¿"_! í)?Þìì\µ½@[œúø\?ïý!ÿ.Hé¿âP_("ƒˆ¿àö¾È'L¿Þ¨,"mb"¿à"Ã`èM1¿Ò|Óz»ÝçAGNbll3FGL J0850.2+3500RX J0850.5+3455?ïÏë;wû1?g,—»‡+n?EfÏ1?9M†Œ?u]'
!£¢?e˜šß£n?ï«´üâü?ƒr)ƒ{:»?@EWu¾?OÈD¬A`?"pFIÿ?'[bsµ‹'?îf}²Kí?Žx‰?v'¢1÷2?jìOL:`4?¦Æ
•J?‹/¥×F‡Þ?ïR¶)×PÚ?u|½zB8?s:·¥qÞ?]³ÌÉ?ÚŒÛÕH@?sBI2ì4FGL J0851.5+5528?Í#wb{äí@CsàâiÀ9ÜE ›€úÀ<Žv3cÛ@|"œT‰ð@]ŒzÍ%¸?²4<ó{b?©ýñõž?õŒSâÖ$@
ð%a¹X|¿±ùiã-¿â¢TˆîP«¿âX._ŽÛпâö²ydp¿ãâÔ}›6¿ç÷Àá‡AGNbll3FGL J0851.8+5531GB6 J0851+5528?ï‹"Ï"o?^b`¡?QÐ"0¿ø?Cý´yÅc?ŠýwÙ±KÒ?€Êð´Ñ?î|¿¿?†•½¡¬=Y?JÖÞ¿æ?\œm±Hp
?‡õ†òïö?"³Øó8@?ïG†à øî?zWo<ŽMõ?g0‰«¨1h?UÈÓy>F?")¶kÛý?x.ԘÏ4!?ï®55bl?f'ÆßI¾?nºÚp?Sÿïùw͹?yÖ6aÈ?a½œ¸Éÿ4FGL J0851.9-5229?åXÚÕ¬¢éÀ˜e"™‡üÀ9·üjIJÀ;~ðW‹@Ë`V{@ä¬{*C?À"'$17°?ª9Ò?ìÊ/ßÏ @	?âTžgà¿©÷؂ý9Á¿ªK̇,¯‹¿êòÇhýÖ¿Ûçœr<¿äÎý>.¹Ò¿ïÿ¹ß	eYAGNbcuPMN J0851-5228?í#z*Áå?°±-D'·?g9;<?`p–ü?¶+\à?×?°†Dž>?êø.¯Îw?¿æ@ ÞÓé?Jn»Ì6(?bñ áDùY?Äօ5Wy?¿½ðòñR?é¤5tÏ9;?¬'×XK?—R"v…½—?†ýàbtÇ?Ƅםòc_?©¹ÿ›œú†?í_NÛ½÷?'üƅ*0?zECMJ³?b,:?³a4í;˜g?'rà""G24FGL J0852.2+2834¿¿ëGC,òÊ@B×ÆÁ#À:]ÎpÀ<‹	%B¯¨@üܞ&H@'[··?ÆBèé­?ÂS7Q¥å?úåW¨]»@æèî–v$?ïÉ,«¿æì-_ߎ›¿å
ñáe¿äˆ—³æKú¿ð?ïê
_ÕR­AGNfsrqB2 0849+28?íÎè'ÑÛg?¨f%\,í?'<<Áؙï?ŸUØmk¿?©óXõü€?¢¢Ýj9?í[ƒ¥2¤?­V¯3r–?^",f1Y?—Ëd—VÉÏ?±_o¼Þ"?¦ç"…&áŽ?í(_¦!tõ?˜xs­ZE?'"í2=MR?'{‰Z?²X'eü?"³'(l(®?íá¨ó½Q0?"ôÐW%ª?™' ÊÄv´?†¸€
MA?¥$ ^ȱª?Š‰#o4FGL J0852.5-5755?Ú5
Cñ' À!	3ã\[KÀ8j$咖pÀ;ÁŸr ¯@uƒ°Ï@J߈'4?¢àÏqì=?¹8Ñ,ØÑ@k"˜€"æ@r'M÷¯¤¿Ùg*±"r¿Ý÷"[nç¿ã·ž'6¦…¿ã¶°@O%'¿ç>Õ]•¿æ²\sž]NAGNbcu3FGL J0852.6-5756PMN J0852-5755?îÄqÛí·? DWñÕb?RÒ{9ÔZ	?L…ê
¶?®M%rÂ? hO&?ï\•ö²¸?§_R¿}ÿ?=‰lÕ1ž!?XCAX
&r?œ>GÔâx?¦ùEguA?î¡r6ã ?'.^¿ë?òà™|?zmՙÊG]?¡s"VY§²?QO½Yò½?ïð&é }$?Pœzöɪ?KC0w‹ß?ÿû-1f?]Ýy‹þBc?P-Ttq2\4FGL J0853.1-3657?h2Ð	á¶Ú@°hÀ9/²Ä
ªÀ;ӆžë2@ ­"Ýõ¿?þüÕ©`à?±upÅ?¯Ql^YR?ü˜.•>Á@ĖóL}¿æ­§"n>ø¿ÛžÔA
aX¿à
fÀÿ91¿Ú-'	'`¿â g߿݋c`wAGNbcu3FGL J0853.0-3654NVSS J085310-365820?è6Äÿñ?´'‡‡Î?'qýY+ó.?uÛÈíÞ ?ÎÈ£OYA?³«Ù¦"^?ãßm–ÛÛ¤?Èü(­ó–
?'äÁŠõ"o?ÞŸ´?×"ع˜ðs?Èdv5³p?ç_@cñ¶?ªlԜ7?›L±'6½
?"m)Áû?Ð.vf$°Â?¨sp3Ç÷?èÏGÓbÔñ?¥êa,ñŒ?¥Dû"Ç?‰Óh}‹ÆK?Çq¡éòÈI?¢ï·BGL4FGL J0854.0+2753¿ìgÞÚÁW@Bóâ?$ØýÀ;þ—ó§,)À<öÀ
¢€@#kȂ»0ÿ¤¢F…‰A?ææPaAcx?ïþÿÝÑ@‹{ɤú@ûëLi»?ã&O?XZŠ¿ïÿßÿY'í?ïöü´>?Áâå¨eå7¿Ñ@Æcüÿš?Ô'»/ìVÖAGNbllSDSS J085410.16+275421.7?êôήé˜ì?Ķ¦¬÷?‡â_I;ç?‹%é@—òi?®ŸOÉ("?ÄfdƑ%;?îjQ4JÊ?°øñ×ãá*?vrw±9þ?Ž€Aß‹?¦ŒÅ3W‹?­ö¸Qõ!{?ë)g!#S¬?¨oMe•@¼?ª½¨n?ƒZ#ú»Ô?Á_· ëÏ®?§SK2â?ê©ÄúÇl?¹¹Zdn†?'‰û÷b¾?3_ûYŠ?ÅS	•äw?¹¹­<ˆž4FGL J0854.3+4408?çún_rðý@D5~g,À:ÎKUhè!À<œ™ì¥°(@ô-.?÷Æ ÆI%
?Ŭ§¾J~?Ò¹]XJÅ@s]Å­ôš@Æm°Ãi¿ïþÞAê05?ïçè絆_?Òç¦læ³(¿Äbl†»ñ]¿çFm!ÁpοÖ5I£bQAGNbll3FGL J0854.2+4408B3 0850+443?ïJmãNÝ?"½ÒEZ;Ó?ŠîËu¯'Î?"þRü–y?Žþ™|¶…?‹ædê®t?ï2-¢n·?˜BâӕúG?kÞjݞþ'?~Úïé·n
?–>~V‰	O?"!Ò­?êmuG€àá?«Å³H NŒ?·Ñú0Bþ(?§""#K?´Â["µúÛ?—âل£){?îŽX4òtµ?Ü¾…3?…ëa†Ã?ys˜û°%?¡ÙØw3:?‹¿a¥BªÔ4FGL J0854.8+2006?ëqQct*@AéÈ!laRÀ7'm¾iÀ;Y'àðp@@Öòj–!@>ü½U`…?"ÏÞF"0q?ª;·²@ºKÛ ¥'@£ñ
ݜ¿Äõ;Uìq¿àÍS‰Ò|¿ãá~ ›¿ãD_÷6ƒ¿æ²¥­Û¿â~25r
AGNBLL3FGL J0854.8+2006OJ 287?ï¿î%1.Í?súš4¸¢?BX±£â^?:WLèØ?}½ìq4û?sŠcÚB?ïH ßI²…?˜.­•?]·L­ˆ-?jnXƟ?•oV¾Öç?—)Ü‰Æt?ï_€"ºf?'/žõçGY?re+uå…?mé‰&?ŽíN;«‹ž?d?ïïpÉô˜Á?N·¬ö/?4d4¸†ës?)ôàÛ¿?\^è¬Á«?LðNe~ô)4FGL J0855.4-0714¿êœeûÊ@7hëíúCþÀ:ÒdcVçmÀ<wÃیƒ1@ÑÑ¿¥ÇÐ@…ïbùÊ\?ÌhP ~Ж?Ø*´ÿ¦"Ó@	é{Y<²@!­ûü:N¿ÜÍ<žÁ̔¿Òþ=Áç¿ã¥Í"'± ¿ê9QZe§¿ïúÞ°ô?ïua Va¶AGNbcu3FGL J0855.2-0718PKS 0852-07?莟Áøo?Àv[=gÚÅ?˜ZÑÄ\?–¾—J?ÊÅž¿šv?¿ö:åùUK?ë¿KNÕ,d?¿Ó§æ²?¦Å"×Éso?³*	.9è?¶¢ãqã/?²Îp/?çá}~·Qï?®ES}0Ï?¸¥L䇻? ]°E¾¨õ?Äw·^°th?¤¯U­ªm?ìt¤aîÃô?¡@z»¥T?"GÇR'6?|`ì´?·HëÙ?Ÿ(l˽{4FGL J0855.9+7144¿çÁMm¤¦Ç@AŸÄ~I±ûÀ:=ʝG¤À<H³B¸u@ñonwØ@§ú D®†?Éæ\Ukl`?Ÿ‹™·Ý¸"?Àe$w®@	"¤èWAÛ¿©…Ðäßh¿âõ°¡š¿èÃÜ-'àB¿ã¡Mø±W&¿ïÿÈ!ÂGŽ?ï÷A)@AGNfsrq3FGL J0855.4+7142GB6 J0856+7146?ïØl Fq€?kýwý€é?Rû—æ*°b?P%R¸¼€?nÆy)Ð?hA~€£¤«?ï^ôÚN1?"±ùY¤@?VÖnØqG?jßQXòò?'´/)?'òËÀZŠB?îRՕk´C?'ÈZ¨ °?yÅ#Înø?koóª¨5?§š/-ñ?@w8®Ç:?ïK4×'?tP~«¬Õ?b4ë˜9u?R@O
c>"?‡_þñd(p?r›»ÀK"4FGL J0856.4-5309¿Ì38bXKÀ3éBNY)À:™ÝLvÑÀ;õP~"Ñ@ "è[ôs@fq%Ý	[?Å%'Abu쿆:¾üpÔ?Ånø_»Q@ÇÔ/‰?éíÊsV8ò¿êѓ ÔÇ¿ç³ß@ñ¿åJZ«¼1¿É24/²u3¿ä3ÝbFF5AGNbcuPMN J0856-5312?Ó
V
d?¿§ˆv%?€Ç?*.Ž?}»†úUý?æ1»·þU?¿ÿ¯ÿØÔF?ÚP¨=Éû?Än4š½†?h»òbœÕ}?~A'<{.?â¾ïî¸ec?Ãþ64Ûá?ä§<¿ÜgS?¯âr†è?›{+O£¾'?È¡ùϛœ?ÔùÓËLõp?®,~¬Å¹?省Zýž?«¸·kç%B?rD+F+¡?im ?Ð~Œ9Wª4?«Û'›™ •4FGL J0856.6-1105?ïÏÚpç"@5y*0U2aÀ8‡¶Šk(À;ôv_î@Ì/E½ÏY?ÿ.ÐG«<?¤r(çTã\?±y¾\òt@T©p¨	@
°4–	Â?æ^Å󔷳¿Øuaµ|¤¿àÙàvoÉ¿ß@dtß¿äÜ&$p¿âF•Ew–AGNbll3FGL J0856.7-1105PMN J0856-1105?ï±Å›uï©?}…r'n?C"‰U'P?@XOœ_T?'U`+þ?|˜²*ºÅ)?ï(¥–'?˜ˈ&ØJ?ls…l0>?{Æ'=?—\ÝY'9?"{ËÇD§ÿ?îÃqxfJK?'Ò«âm?}Œp?z¡z± ? '…ˆ
Y
?ì)ëïwµ?îl4¯F?ÂøýZº?ƒÌZÕªNÜ?oKs™áE{?¤C
wç?Œ‡©—Ø94FGL J0856.8+2056?ÏdÈõ…[R@BD™÷LÀ9úÑáÃôÀ<<FipÜâ@7"/M>@'q›MÏ?º á!§¼?w(ø¿n?âÏbcøM@H[¦™Ý6¿ïÜô‰u?ìýçՒï¿âå‰\4´=¿â•€/eH¿ÝÝkëáe
¿â\&$pAGNbll3FGL J0856.5+2057TXS 0853+211?ïs®Àˆ?ƒBG¢vŠp?fˆû4Êî?^ZڒxÂ'?r<«>]?ä‰Þ'?°eŽ?ˆ•`Cû­?Là+š~X¡?XÌ"P¸Úø?‰'Q,ôs:?†Ãæªeõ?íŽ	bØAì?–?<,Ëe?‡\¼¾äk5?{;Ÿé
¤X?°¤Qac2?'ÖZ õ'?îÎx¯tÇa?'d²êÂÀ?"á.{0?op'(V?œ#yz)KÛ?+ÈF¤q4FGL J0856.8+8559?Ø<%{v@=(dŒq"À;c~h»«<À<¾¸‡›jT@·à™³Dæ@'ÉÜW"K?ÎÓw¾RŒ?À*ךOJ?î*Ö7¯™¶@Ň3:•¿ìøžï!‹?ãgc¼gú»?āBJR^¿çw5<滿àÆ7½¯l¿Ú¹9±ÊéAGNbcuNVSS J085740+860344?îÓaõæ?›¤uæ0 Q?Y%PÂ]Ò]?Qßç'Mµu?¢¶(˲÷?›EzA	‡?ï{¾¶ž¦ì?MlÐt€?QÏÏnN÷p?eR{Ñôx?ŽÖXjŒeæ?Œ"u§Fù
?íùScê[?'"GLß?yßÁÁe‡?nU…(ˆ½?­.ї_mœ?'K߂âO?ïR ^aM¨?z"ƒ ¸Z?`F•óî´±?UTéÜIR?"³!uXt`?yÊeOº4FGL J0857.7+0137?æ=]ĉåÐ@<™;ʸÀ;8ž'7À<‹m{-È@…9C¬Å@tßÔŽ?Î.†¦!è2?Ëõ%Ü]Ž|?úPÞªDâˆ?ö¸Dý?ïðÓÊ¿Ç""FZ¿èˆóß`MH¿ÙeNëž¿ð?ïÿø¨ó©°AGNbllRX J0857.8+0135?î ­wòÆá?¢mèþ?…Ìhtâ8?Š¥
"þ? °5f¶YU?žw1pxØ?ê–kTbk¥?ÀSeƁ?±f0"•C?·øڝ@°{?¹ætÉW_¿?°pIémÚ?ë>¸vMí?£R~Ñƾ?¦æÞzíŸ?"ͪ^c%n?º–ÍÕ?¸ï—w?é_ê'0æ…?¬«Þ2*‰?·~äž}/?£`jIÒ?½í-	ÚN£?¡ÉþáÉÃ4FGL J0857.9-1949?ÖNʤ¨@0‡Ò"œ²SÀ9`ây|À<kc%iF@-_«·@'ãt®ÿ?¯©.Zêî?Ÿ¾E†®¹?죦-%Òø@6rÆÆù?ÖÙo]»¿ä¤øÝÌÏQ¿çH/^'\Ž¿åÐZ‹fÐï¿æ…bªð3¿ïÿ‹›ªAGNfsrq3FGL J0858.1-1951PKS 0855-19?ïÞÐ#¬)µ?gê†Ù6ÿ?Iãìôå
¹?D0³Ûژä?j¶áÜ?e§ÕÞ?ïÁL¸Eá?ƒ"0ó\p?@Gz.gÌ´?Xµ"(m¥?}hê^'?'"Eo?ï¯bb}?þì@5e?tsÂ!œ|?gFÛÊ|Ðö?™)vΫIQ?}x©EW?ïÕ.~V"Q?\¾˜­g?SÜØKÆÒþ?B(ûî¦Þ?pqŠÁÄ£n?XO½¬Á1Ì4FGL J0858.1+1405?í¼ÎNõº@A.j¨ëF5À:¾ã²Â_ŒÀ<oy¼"€@:ªÆg­ä@y\ã/å¡?ÆŲýî?½Ç;¾G"ÿ?ð"X6ù@±øÀƄ3?îÍÑ–0¿Ï­ò';׿è¥8hýœ¿è®½>¿â%Á?ÐÐh¿ïÿý¡UûŠAGNssrq3C 212?ïŸ>m¦ù ?|Xÿ.5™L?e[à$'ëd?cW¾Tß8?'Ùl Ý~?x¢÷‹À»?î¹+û¤Ùá?\QäåÆI?q()Úðb?wñ~P?¢H;
T_X?š¡ùè?í/dÑEd?—"I[¹m'?"›³à48?…º–˜¯?±rˆßË?'âVZ€?î¼=ƒT?Œãp"6?–­é^?'êo²'—€?¤åå_ÛC?…‰­¾Þ4FGL J0859.4+6218¿çpøiø[
@CDhۋ¬qÀ:ÀõÄ<ÛSÀ<±‡O:J@4·jºÞä@WdU/?½åœQ"×ì¿}æñˆTC?½ðÆQ2¢•@u3`œ˜?ìžÊÆbO€¿Þ—u;Ê¿èú'`åóå¿×µ£euP¿ç§ÛACl¿Þð?ãÅ·°AGNbll3FGL J0859.1+62191RXS J085930.5+621737?ïýtÆ3l? è—ZÉݳ?\Èãi~Æû?_ëss¬G?ˆg†aCL1? 
ÏÍî.s?ï¦óoä?'Tà{=?AÞ9 "|?Q¯Î¹(Ýì?…\Ÿ'´ö[?V0ô¶G?ï
·Ê"?ƒ8÷ïÞe5?iÁ<ÎeÕg?WEZ;Y‹?›"ÁlàÄÞ?' cñµ?èü?maò0ÿО?k?jL[$,?Q²D'îè?"Šárä·Ð?jxcë@çº4FGL J0859.4+8345¿îîxð{@>MÊ:KUiÀ<êäåÈFÀ=5ôÆ/@"˗‹!†¸?ö¾0'}ó?Õª• Õ`?юcpàÓ?÷ÄÉÉMì@ž}"D¿ïÿðÇô ?ïùªæÈ÷U¿ïÿoì÷å?ïþ=BUºó¿Ñ¼§›dõοáñ@ÅÂíAGNbll1RXS J085916.5+834450?ï'C`ÜÌ?Ž¨š~â5ö?] RÛ?`Tç[®á_?ˆ
8æÔ?Œ±iᘦ?ïŸ#Ë\ƒi?Ï?1£É§?KDˆ&tæ?h4… òƒ‡?†'Ħw×N?‰¾[ø¤Ž?ìÞµWÆO€?žr¾¾ÞQ&?‰× õ…è?'…b¡ö ?µÏa#ã(?œNŒÖ¯äË?ïBãBì}?ŽR•¯Úò?gڌœë{×?r^`¯º.?"Â2º?‹ƒ~xÁ4FGL J0900.6-7408?ïªÔž—.À1úgèF¥×À:1Y³Ð|…À<7ä¼­šØ@~Ë?"@¢ùà0W?Şԁw
þ?ÉhÚÆ_ ?üö*ÿˆ
ü@	}Ð3´f?àbù"«ô¿ä~Áï#9¿ë¦°8Aí¿îg"¾Ái¿ÑAÿE¿ïü-""ÑAGNbcuAT20G J085959-741401?ïîŒP˜{?i娲A?Ez³"u;?T‡u=ɕ?X*
¢@x?dC¼c2?ïh'ëé[?˜,h["¥t?X9œæ2|?lÀŸMkæW?'{Óú"qw?–~Šüö?í‹ZǟŸ'?œÿ㐚ïÌ?…ïCԖ7?|و6o[\?°çAHpAx?šgsOð?ï1øè¢?w)é}?cx÷^áÊâ?W«@Vw?‹UD dñ?u-±Ó	õ4FGL J0900.7-1243¿Ö&
Žf"@5SÂCÜΣÀ:8èí"ÃqÀ<`ÎùͶØ@ßڃïŽ@"'A?ºh…¥pè?˜tŸ¡?ß"äRzv@VÞyzÐ?ïÿÞ§À£Ê¿Êši7Ñþe¿æÀŠt8¿â-%Òø_ù¿é-"BJ'k¿Ú&$"AGNbcuTXS 0858-125?ïÌ̖óéÀ?xr<C·Xà?I¸¡ÞO:6?F»•Üí¾‰?vb JA8†?wQÙéìZ?ïÆ8>#»E?~-òÆEü‡?8Yà\ÖP‹?LYO¶ù5Ÿ?{^BèTø­?|§G@ɔ¶?îÉ©B‹ü†?‰ÂMÖaÙ?w¸½~@'Ÿ?pÙHP؜=? nT'x';?†A^Šx…?ïÔ'druæ?ZôrŠŽ?Il÷7¯?5
BႷ?r¾®ßÏ*m?X⁓Wε4FGL J0901.2+6742¿Þžh3"@B‹kü¨\«À:iTK±¯:À<cۖ"+œ@¥À$Ä!@rü¬Žhä?Ã_5'n·y?Âf‡s|O?üvѵ(@ ov°?ïõ8ü Ïï¿âçí_>~ì¿çÃPýsˆ¹¿ä4ÂI¼´¿ïÿ¤€RuÄ?ä‰áàÛ!¤AGNbll3FGL J0900.0+6754TXS 0856+679?ïB‰lXP?'ÁƒR3«Ï?Þ¥‡P½ô?D'F§÷?"h\̗?¨`w–ý^?íïÎóï¶?¨½Yɲi?ƒqý%âv_?‡ Vt‰?¬&'wŒ°?¦ú`¢<ê?îQ© š­T?«õÑ;°Ô?€ÙÉV9µ?r š•˜N^?¦Þ¯ƒÿœS?Œ0¬â¦˜?í®ä'Ûï?'`λºÇ?š–WÉï?'À¶ñ'~÷?§Ôã=V\?ŠH¬jcš4FGL J0901.4+4542?̊4e§˜@DªV"uÀ;É«¸€®À<ï[:¹9r@ù"D›?ü‹rX?á^$Ñq?ï÷ÝâsÓ@$ †å@í?³õ¿áën"cÔ¿ÁÞ/5L½ô?í_«–òm¿æwˆ,‰ËÆ¿ïÿԖũÃ?ç
ò¢IlAGNbllNVSS J090208+454433?ëÝ7ÂÝ	ð?¶aŸˆç•†?¦oÓ¦j†ù?¤Ç?·/­?µÞXâm?²SÐÛ
z>?êCÀ°¸·?äÛwÿ?²&ºØ~¬Þ?¼w-?åæ×?»¼¿!ûj?´Æ‰u¯A½?ç§@NM&?«ðÀþ9tÔ?»fM#MÇ
?¡;wDÕ‡?ð€mçà?£¤ e"þ?ë<AzÞ(7?­-'•@a?£1<ç¶í?£At÷RGÆ?¼ÛŠšâÎ?§\T®;i4FGL J0901.5+6711¿ì~V[¯¼@B¥Ÿ<pÊÀ;>Iç«À<Ÿ.X•@ 'è(ó¿*@´{'G–?ÂÝ`t#"¿…ùN'fn–?ÅúöÖ¶…Ž@æ"Ïíú?î'"2wL?Ö"D"™³¿äx7ÿ˧´¿àõ½ò>v]¿Õ¸"þ<[¿Øæþ§:l
AGNbcu1RXS J090140.8+671158?ï?™eL?H1'ñ?gNÚ9ôaB?`ÜaA?š®A%"ÊL?—Ă?ï^í+Ô|?‹ˆ…ܺêM?QJ%Ûkþ€?`="
 q?"'ßüΰp?‰gÿyÁ:?íÿÏí&«õ?'ìÎ2É?w[
lÐ?e¯æ«'˜¿?­Ÿ‹Ç¦²?yê=ë·Û?íýoÄå\?'í.(d˜0?µJCi?röêl§X?¬2nRaÓ?'æ¹Ɗ4FGL J0902.4+6440?éÆæY÷ÔI@CàÁvWuÀ;A&"Ï:À<ÂFÊ¿¬S@ǯ½ó@)@ç*໗?Å°'åøý¿ OáGÎ?ÖùDåè¨@ïƃ°¿âëE=¡Ì¿ë'} <5¿Õ1e¾àÆ¿ã¸É_¯èæ¿Ü¬W¿ïü­/x"AGNbcuGB6 J0902+6444?ïqÜ"på?Œ:À¢~Ã?`Î:"/ɵ?VÏŸi ?UhÛ:©Ñ?‹'\"ûß?ï"Ûàoœ?…yͯ'j.?=wZ"à4?JuÛ ¿ZÛ?Š3½f?"Ûí)žƒ?î@ƒŠÆ?î¨Ü_š›?€ÏÉú,Y™?väF›×ÂÙ?ª˜©<=.?®é&{ò?ïc"–?tšß›ºS?U%œÃºÆæ?Hëo0éX?ŠƒÂ'1?tJ|
4"4FGL J0902.4+2051?éUSî@BàûC؜åÀ8ë+•°À<út¥ÄJ@𗏩*Ü@ã`dÄ¥·?§ŠI€¸³L? Ä©H¹,?ö;ßßÏ@hGn~Ð¿Ò<Àåä¿à5Úã1¿âIšHB‡¿âTä(3$ð¿àF4—·AJ¿éE‡=÷\mAGNbll3FGL J0902.4+2050NVSS J090226+205045?ï¿kÙû13?¬
-u I?B!¯X¬²*?m…4t¢­?~ÝQÐè?ª50G°Æ?ï¤Î÷}°?…±–‹ìì
?EgË¡*iÀ?X°Ä8õCÚ?…uß
í'?"›¿~K­€?ïBƒ 05á?~ïÑm<è?hÅñR›N;?Xñ—!Ú?"–ÍÏ¥Ú?{¦"œ¿ìµ?ï×ċûº?^ÈÂ7+?Q4Ä5£B?@]5׃Œb?o¡sés=?Zå¥Z®4FGL J0902.5-4801?»6í+UÝò¿îÃ"N®ºÀ9 ìt2À:ÞÿÕ8@›ýèx¤×@Q<\§¡?Îãî<Cñ?Üj¹œÄFk@Nªß<;?úi·¬T1[?íD8¿HB¿å¯m@u;¿çÐÓDM¸¿ìŽæbJ"
¿ïÓ±B'±v?Æ4Ü5JAGNbcuPMN J0903-4805?¹Jò9$YŠ?µ-ûôĶ?³×r;ê£å?²×©™µì?ê[³q^ S?ÀÀ
³{x?®"~K¸˜?®‡è©Z—Â?½©­áï`w?»²"?êb'_‹×?»ˆz±‡?Á¯æz8¿Ç?¡ÍÙç_;ø?ÇQ'Ú}¦N?¥Ã——)am?å¿¡êÒf{?«­þ>I¹?'#Üj›
?iÚؾã	Ü?ÌhÄF1O?©§"ßZ¢?èB"|É@?©%Mj±È[4FGL J0903.1+4652¿ï(tJL â@DÉ}ke©¨À9ǽWäÃdÀ<{¬h©6Æ@òS™Z. @üc®%AÙ?¬¸9lÞ$¹¿¤€ýbäC?ö‹‹Ÿe@zêéz¿ÚÙaE?OK¿åÍ:°ÕöA¿ç0[b&eÅ¿åtáTù׿ÞFãÿ™RÍ¿ìàÁvWu2AGNfsrq3FGL J0903.1+4649S4 0859+47?ïŽúŠì#­?'FE/6?aû­~'¨?V3t¼'?‡Âqåm*â?+¬ôAHf?ï`>`ÎÐ?'؉÷·?Sêü"'ç?a©'Òe6H?'¹"$§Ã«?'!™NË?ï
!"*?…À:`áΜ?n¦¡KQï?br⹯ ?šíLJ¤?ƒ'eÑ΍3?ïrÇë¡«Â?x>^Sõ¿¼?zÝbš\ô?i²¦¥h[?…ßTÇáy?rÝñÜåá4FGL J0904.0+2724¿æUÌ",ûŒ@C÷Ä"`À:E®†¨YÀ<|Å<µ'ô@ïIp6t@~*Ã") ?Á—ø¯©¦W?ÆO¬e¤®?ÿ¿ôw5Áƒ@	¹H~?Æ]B Ç¿ç§"™2¿êß"²¿ê§}½›¢¿ïÿÞr¾"¿é´á¾ÌY
AGNbcuB2 0900+27?ïѲžÀh·?o¨Ô]a?hþ¼L»®e?d¾Å·Aç?eN¤òۚ®?c
9%r½?ˆ;¥?¥y9|[yß?xÁ@DÛÔ?ƒëÓþÃ?¤žÿwPË2?£—)±?îÁð‹'æ?‰¤1"[{?€ÿÙzВ?t,üo'Wx?ŸB'%ZO?…ƒXãÜàî?îÔ¤ë­;â?ƒðµ~|V\?"Î́	å¦?}ï¿U{ñ?'œ•	Nž?u¤J/¦äÞ4FGL J0904.5-3513¿Æ̧ç«@<Ù|ÞwðÀ9cЗ\¨À;Ô¯ÂÐʈ@'º.9¤<@¡&cAø?¹VÈ8¾b|?Ä@l³sà@#xà¼mÚ@.="‡¿Ì
#)$çk¿çw9ó@ÔÜ¿ãঋ(¿ë2O¨´¿¿ëÛÞ´UÞ?¤@ª; gAGNbcu3FGL J0904.8-3516NVSS J090442-351423?î¹Z~¸°u? ¡^ÊõÒÃ?v•¢Ž«{Ù?yÒ
ª±-?¡—£ÂŸ‰:?žvÆns"?ïL½›C?¤üB"ª§?NSY™Ë4ã?h°wߕ…z?›ƒÍÉEw?¤Ìçý¬³Ê?ís+_y²]?™o¤œøÔ?'Õ³ÆßØ?†·å{Xû¢?¯âp%VjL?"DIÙé<Ì?ï•n–"›?qÞKnF™q?Uaãä|C"?B¨¦P€I?‡øâMÀ?q^n<Ɵ4FGL J0904.6+4238¿íc3'¹æ@Dø<÷TÀ:Ÿú D®†À<¨¦tsoc@tTc¯|Û@ôóg°?Ä©À˜¶ð˜?ÁǶb}#?úOSû)×?ùA˜‹Ò† ?í@֟^'¿åIÁêñ{¿âpŒû%¥¬¿â}5€V¿äpŽ•·¿ïÿï¿@PAGNfsrq3FGL J0904.3+42404C +42.28?î'$<îOÖ?«RÚ{z?‡{¢®7(?¨?@òQY'?¡þÓ©otØ?™šoΆۜ?ë¥c5êq?´¯m¼Ý½?¢#RTYÛh?¢ÃBþ?¹Å«¼#¾Ä?°°ù'Ëdú?í‡cÃ}š/?"I:¼âE?‰}/4ÜL?x»ý+'Î?°•;ýw®3?ä5uþÄ=?çù–[2"ù?£Âiý5Í?¹qm.z?"ƹ˜À!?Ãa\žäã?Ÿ'±eëÐo4FGL J0904.9-5734?î'²¨xÀ$«>݋aÀ7ÉÜ_çÇ$À;IŠ]ÜT@©b"@Úºp©¶?˜#yç;?¥´t€b0@
6lmçd(@"›æ¥ç¿xÇ!€òól¿â$Ÿä6v¿äFÿ=T<¿ãw÷*|«¿ælŒñ«¿áÛ~ AiAGNbcu3FGL J0904.8-5734PKS 0903-57?ïؕ°]L?—ÀMfZH?EìOiÏÖ?OèôoìŸ?µŠÎ«à?—{Í"¬ü[?îµõ¨(Q¦?°ÈL€ŸW??îNa`YÊ?\HI=ñÜj?¤`Èà¸$â?°fÉÓæ?î.ÐÒø˜?–-¹Úƒ­?ˆvó>?s³ç½Sç?©.¤p.²?"9´Oñ˜?ï󌔻ì€?I\´ÁÀg?BïvÐä?Ó:k+¥|?W§'}?H¬l0æd4FGL J0905.6+1358?ÆÓá¥2:@AûÚ¾'œÀ9PvÄ À;Ì(Hôe˜@:grÕàr?ùv÷xr¥?²‡›À:m9?Àk.¢)àú@ll—ØÏ:@
õÁòSD ¿Ú½'Æf>¿º{Ýñã1¾¿Óžœ"_ü?¿Ñƒ%Nn"¿àäëa¸VÉ¿ànÀY!AGNbll3FGL J0905.5+1358MG1 J090534+1358?ïÔ¬V"!?h·‰ž7ã?\½…y?o?X`R4D?lôç!?Z-?b¹VÆ*"Í?ïLŒ.µˆ?'«³®?aš¶¹m¨?n™k·=[Ô?";#R!IÒ?—Ða©]?î҅±%¾?'GEâ?·À?†!ççѺu?…µý÷Ie¡?šžUê'k?‡±¤ƒÔlÏ?ìÉȆÚ<ä?žDÑdŽëV?€Ê™+ªã?i‡¶7¢¼?·˜h£ËCƒ?ž|~\Ößé4FGL J0906.2-1707?îïT«°·@3¾G'ܾÀ;"æ>ÚÀ<l»êý9@ x–†>Èé?þ0M:Ev,?ÑÕn'€ñ?È;™¼)<?øääÖ®ÍÞ@4ô‰)^ô?ïÅì=«\:?̵FÞ¶¯)¿£O.D³Å¿Ú>Ù#ó$O¿àœ¨AÓ	'¿ïòË.g˜AGNbcuCRATES J0906-1706?ï~ò`·òs?…Áƒ^­É?\흓ÏeÅ?W¡ÉE'¨?Œ¥´‰v…?"¨'•Ís?îC/®¼¹?§({2pY?u"Á|us'?}2=ozuÀ?©dՅ…í?¦?U@µêŽ?íÒJI"uØ?'6'wauZ?ûph`e?sÞÇ\žÂ?®\w‹žŠx?}ÕÐ?ë±O'@ç? èS`O¦e?"cBÛ€?…—î]ì?½\¶8ƒ3?Ÿ
àø'E~4FGL J0906.3-0905?í'J^Y7æ@8'sÕº²À9óÿò"³À<Qäþú2@]oqÒÖ@^쿱[W?¹*³Éƈ?´sßrkØ?ûåCÃC@‡-ã"ã?ï;ái\æ?¦½nú£¿ÝÞa_@'Q¿âØ)Âq)8¿ç!½T‰Å¿áŽýÉÄڐAGNbll3FGL J0906.3-0906PMN J0906-0905?ïñ—\ÏØ?V×/z"ê/?0â›ôÉː?+¸•¯ü?X˜Ÿcdn?Tm+²^±?ï¼&NA…?~ròáM?9܎bÛçO?HÛ`‡ùª?€'‡ü£?i?|ô»½ž2?ï'ýÚ^1?Z¬Û&G4?s~ƒ1ؙ"?o¶YD¯Ê?˜®x>™?|ù£ñgÅ?ïÁi‰ùÏ?c|¡"™?[T0~‹u?IÙë4¤›w?xke÷Qõ*?`³'B¸Íp4FGL J0906.7+4950?èíToÿþd@Dõn?x»ÔÀ;•X'ßBÀ<ÚpΟ4ä@JÏß%ë@RÈqz?Ì\K‹*¿Kñßő´?ÐØV"¡jž@*6jX‹?ïýùà¬'¼?ÈÅq¤2#ê¿ìâ?z¿¿®UÙa–Ú¿é×»]Ž¦v¿ïåj‰
ÖAGNfsrq87GB 090322.8+500444?ï©°ÈK‰?…º`	ØV¤?f"J",@‰?y­bB<»?ÝöÉ^Y?~
>`æE§?︀ž#ß?'©öDŒh?8³†¼DJ]?N+oYWÏ?3¢"æ?Â3E¶Ÿ¾?íô5o$2?–ä)Zⳁ?|ÃU¹öY˜?tdyÅÏÆ?­$DAÎñ§?–&ÌmˆE?ï¿è®}0?m]>[E´?b@ž±îâ?YßEŒZWÚ?v맜èq?fŠ,nGÅa4FGL J0908.9+2311¿ïf©EšO2@Cô$_ZÙjÀ9ܺã–<îÀ<%˜°eù@ çW˜BV'?û
RH¢0A?¼Âs,lã?»óÈd2Z@M€ÿnàˆ@[,þåÑ?ïÀ¦]ø-Ï¿ãIJh!R¿áŒ…0aÈ¿Ôð¤ÃCa¿Î-)ÙÃ*b¿ãö9þ(kAGNbll3FGL J0909.0+2310RX J0908.9+2311?ï;M	û3¸?/ô—½ðˆ?`¶Sä÷š?g6¨îÆE?–"§öê?ŽÏî9?'‰?ï'TÌ$Z?–o·Ýý3ò?cšTøÛYx?ru4š¢€?˜¢2`	"?"˜ÜNÚrG?íÁ«"óÌf?˜Ÿ
Ž[Pl?sòî5`?caWj®î*?°³xŽFÇ?˜˜¶Þ4?êv¢–ôä?¢*uIJå?‹®>H@"‹?{uú«XH­?Äj'¿«|'?¡ôÑ1¶
4FGL J0909.1+0121¿í©.·ùV@>í/IŒ;À8SÓíçÐÀ;¥­'ž"•@Á˜€iò¸@ì´^@ý÷?žT©œéQµ?¹_¿p@
¿ó v@ð8æP?î‹#Ÿ—_ƒ¿ã¯Þø¿è>þ#†î¿å¼Ù¿úVs¿êìÔÿ÷«¿ïù0¾
í)AGNfsrq3FGL J0909.1+0121PKS 0906+01?ïÎì@]³&?pQΫ‡'V?gÛ¥³o…?c¢'$R?i8£ü™i¿?cdmC¹÷?ï'yi"¶G?ŠBt§—,?Qw†¢àFã?`¤Úw\q?2´Æ¶e…?‰&ˆ—Åö?îŠF¼´Uo?•U \̗F?,NA•ct?ˆÏðèS°,?Ÿ!Hª ™?¦n^¶Ïü?ï¶ÎùŠ2ñ?qgô|-½?fÙڟMU?[û±<›ò]?y+ó͖às?lšø]Xj4FGL J0909.6+0159¿â·Š(kÅ@?\œÃŤÀ9DkHMwÀ;ëÛd?D¹@"ØБ(@ZÜ
²p?·` SÇþ?¿äq.@…@Õ"Ü£Ú@e骩}¿ë"ÎÁnŸÆ¿ÜQj€ÒMj¿ß;t€¿àW1	G|¿çDP'èË¿èx¼_eóAGNbll3FGL J0909.6+0157PKS 0907+022?ï&«ÿÌZ?š®bâ?rJ|6é"?j–9NÁBg?–—ûþ˜º‹?3š/L?î4hÅ$È?«¤‡'Zx›?Œ\¤ÌZ«M? JÛLJ«%?§Õ@—Ÿ? ñ<‰³ù?îqŸøPà?–Ã%:¸?ÍŸ‹R7?uYþ†²Ò?«5~¦m=?"¿•K3jÉ?éÞ&ZZÅ.?£@eѾÚ?ª`ÕXK;ò?aœ=í³?Áï1@'J? 	ëä4œï4FGL J0909.7-0230?îŠåæh@<þrÚ/­À8'æ:\aÀ;ƽÀÀO@#êç¿í@@Ñå:Ü?£+w'(ãÏ?¹ºÙ…AóÀ@mmÁ¤{@K¸»÷¿ÁæƒA¾fX¿ÞOX,翗¿äÆÄ	¯¬+¿ãò<'Î{¿ëùÍNY¿Ù#''%ÎAGNfsrq3FGL J0909.8-0229PKS 0907-023?ï"Ç.4o?ˆÛƒ!«9Ë?irlLˆ¦?i'ÜÎêVº?ˆq !Pºx?†!Eþ֏?ï/^ÐBX¥?™´»–ê!6?i{ÝîVz?KƒÍº]ƒ?–äª9ê ?•+Û›Þ?í‹,½~v?¤=ŠÏôà…?—à
"4æ|?'&,¿k˯?«]-¥e? _B;‹ñ?ŠµíR?pWSM´Bå?qNÙh¸;'?_¼«²ŽÚ³?'mðž(œ?iË%æ"^'4FGL J0909.7+3104?ìU¯kN5@DõË£!hÀ;PKúˆÈÀ<ÎañŒŸ¶@ 7‡bàJ?ýñk—þŽç?Ë£ƒè­S
?·ÑêK¸»?ì[›Â=Ҟ?ýž…´Š`Â?åÇà~ÛRL¿Ñ›Dß­úû?ÊÛÿ…0Öâ¿àxzЀ¶t¿é6añŒŸ¶?Ä]Ý@bp¸AGNbllB2 0906+31?îÜÍ/—3?—Ǻ­•È?gÉþüQ?f/Ô|ÇúÓ? ¶›…nM?–ÝWû£;r?î¹!—? ã©é^¦1?m¦ò4_…?t"Übç`?¢"KÍå"?žêÛuxÝ?íÁo^'²?"Ÿ+ï?†ð?…P–{+XÏ?zïᶥÇ?®šSkLþÎ?ÓÎù"êÝ?í­5Ø1?"ó߄è½?‹a´c%~?|yPÖЙ6?®O¦9³s?;ƒ-]ä4FGL J0910.6+3329¿ëËÕEí(@E;\B 6À8܈'=À;ØÆï=:@¨Xx4?þn­È$Ç`?ªˆ͝‹?§yê&Ï͈@ì6Kìh@,ñê­Ø?ïõ@YŠ?Œ²QUø¿áS£ìó¿Ù
µà¢Á¿âêÑÀ&¡*¿Üj5"_õAGNbll3FGL J0910.5+3329Ton 1015?h.Ðz?€n`·æC?UTdÕy×?pöüó>µ-?†ö[g±2^?{w~¡ìšö?î{кÜëº?¢²>MUP£?zø»Z¥²?…´¡C"\ª?¤ãÜæܒ¦?ŸÿÐÿ?îxQKÿ†?"³uÀÔ8?vVáM=9 ?q®‡Äå?¥°$X`u?'úºÝ?êâIºÓ|V?£´~Ì~"?­ýu3°…?•7˜ó
Õ?¹î÷ŸJE
?›ª?ŸÞh4FGL J0910.6+2247¿åWj"¥Ž@D;`(^ÄÀ:È­ƒ[jÀ<£_ëøâ@Fá'+¼@Œ—£TY?·à…;h¶Î?ÅlÉKR@/–@HÅl@ÜD!×?ÁâIá n¿Ñõª§&¿ãTגùlh¿ã·#240¿î0(QWáh¿ï骝i2AGNfsrq3FGL J0910.9+2248TXS 0907+230?ïA5A"H?Œœ¤R¦r
?|Cs}¥Z?ue;{¿?¿<xˆ-~?ˆ*7ƒ°5Á?ï=àÝá?"ûÔ³KŸ?I'DN(Ï?^oDžòl?Š©|Båú³?"|ÅíûøÐ?í]¸S»³?š4^>¤¢4? (Œg?Ë?'Ò ~ï
R?©ûòS…8??Ìcì?ï"N˜:?rz6b|B?Y##­qJ?HÎk×¹ô4?ˆ46·ƒr?q[Ŭ¹LK4FGL J0910.8+3859?À¡H(ÂR@EáŸÂ¨‡À:Céœç+ôÀ<‰>xá"-@1o¦Öîå?þ#êÛ«Œá?½R'KÕÁ?º<kÁ:d?ÿ	9d¥œ@
PÌG@Ü>?ïµ{™>¿à6]õ~œ¾¿ázd ¯…¿Ó>.#~à0¿æegʵ¿åšQ_™¿AGNbll3FGL J0910.7+3858FBQS J091052.0+390202?ïäá7OÆ?\±›ª/…~?7­ŽGÚ4?(¦¸*¡LÁ?h)HÿÍýê?[k#±ï:?:Óµ¤?"íÙ²kG?GÜ͇ôõ?Z‡l<%3?†¡"~:Å?ƒ@ïi[Ïï?ï*yìö±?€'²û¨¿?f«þD¯Û?S%lÅ®"n?—éÐùËHB?|ꐨ2"?ïXü°E?tªŽz¹?r¿Ò(­5™?WÜc!üÃ?>ßÑ*?rFnPÂåo4FGL J0911.0-5047?¯'L²¿üð¾'dÀ9v,:ñm–À:åÉêpL@F\…¼íÝ@Œã›EkD?ÃÄxÖ*š?¥
$:qì?æìË:%•¼@s]Å­õ?îoÚê¿äÍ]"̃¿êL!@Âgï¿æ÷ ÈÍcÌ¿ÞMŸ½~ü¿ïÿâ¾÷!AGNbcu2FGL J0910.4-5050AT20G J091058-504807?ëîçÎ߇?¶é9Ó¯Lž?f3U{a9?cë$°Ik?¿Ø—î[ÈÆ?¶§Ù0yª'?ÝÂo'èÍ?ɵbð'»j?måC&Uì;?}Â쁑¹?áâûÒ5­?Éy¿ÿÔ?ã¯!ÍóEÝ?³nD%14? ß¢Î,ï?‰ön9"ö?֏Ào¿®¨?²AÁHÛ÷½?â?/¨HY;?³ùV?wù€‹Ú?g3N]ÑB?Û!º¬úÏZ?³yY|¦ø4FGL J0911.7+3349¿ã…x;"Åc@E_0"'À:}7褚À<FÞ˜¯@1{™>@…¼‡Û+4?¿Žù£?ˆ™õ'œWî?ˏà³3ž"@Gò[§›?ÅïšØL¿é,*?ï"2¿ã®"&±¿ãhpa'ëO¿áRG•ÀÇ¿è‹Å .AGNbll3FGL J0911.8+3351MG2 J091151+3349?íÑjÎZE<?¡‰5ËÏ?€Xüphjx?tà힚?®ÓþA'²? @êaæÏì?îú÷ù¦	ö?—'_=Õ­h?Y7¥:§?b*¨RC&?Ÿ
†yÍ
Ã?–ÌR{@·*?íj~tR;—?–'E¹\r¼?'&§âgþ?j±J#dÄ?²hçˆqÖJ?"Î$©u°£?ìc2¡ÿƒÏ?•µeOl+¿?†yrZ/{?q‹Ðª%Û?º9¸›—?•ø¤pd"Ç4FGL J0912.2+4127¿ÕÇö…5ù@E«ž¾œˆaÀ9ÍÆÇÐÀ<cJw—@¼³äsˆ@\±×?®žsóí£?¦-4@¤_ñ?ñäB"ßÎ1@€"[ï¿ì¿ÚÆÁ—"\¿âµŸSí½Þ¿èܦÿ³©æ¿ãµZTà,%¿â븮㮿ïÿAÿ~ÐÀAGNfsrq3FGL J0912.2+4126B3 0908+416B?ïò¦tŸP?Sò´1¼C?6š%5¥ûÈ?2=|¿ÚK?U
KÉWáE?P0¡ì4K?ï¥ÝoËÈê?&P¶NA?:£ƒôß?N'BºÚ•Û?…³‡ílí/?æ>õÂ{÷?ïI6›F{Á?{B€Ê£€Q?ihÙïk?c›E‹²É?"¬›òš?x'ÿw^÷?ïü""mµ?+ò^…¤°´?L›ì™·¯?šâ[ÏI?7ˆ5˜Ûãµ?)Ã)ÏÍâ4FGL J0912.2-2751¿íÝ:in"Ä@+×ß°Õ À:w©"ÉÀ<´9Xb@(½Ã@Ë—¦zS?ź†c±Ö&?ÓZ]-W§@
"Á{_ò¯?ýæϧóyŠ¿£ÝëœàdÉ¿Ý»÷<Œù"¿è_}¾ò™¿êL'ÅA¾¿æʳ¸(ÐÚ¿ïüƒ]œ"AGNbcu3FGL J0912.6-2757PMN J0912-2752?ágxü=ÝÆ?ÃܑÊ5[À?Ëk'-G1?Àž~¡=Â?ÏO°|ÛA¶?¾ì:Aªžü?Õ#¬|!y¢?ÊH6Ẏ?Û¬Då4—à?̓~=z°x?Î`=SÜþ?Äl½Ôš(F?áT'Ê¡îî?°Ö›k»
?ƍ&­ûE?©£Ø'W
&?Òg¾Ÿ?©êD;ú›/?Ò¥¼,}?¬¾:þýõE?ÚFŏ,Ý`?¸ò0÷?Ó%´§"#?´kžuÂ}4FGL J0912.2+2800¿ë0ƒïŸpÚ@Dìä¸{ÜðÀ;REå"TÀ<¸é_ªŠƒ@!þfUõU¿µt'ÞÛ?æ$ãåF?ïÿÿÊPË@Dʄóð'@Ô«-•º¿ïýH_ë""?ïÿå"m/®¿ébP¢Yܕ¿álpk¢æ?âKYÎy¿åÍ+Í
dmAGNbll3FGL J0912.4+2800RX J0912.2+2759?îÑo0/i?°eµSæ¯?ˆG¢nȼ?¡ÛOHŸ?™®Lâ–?¨k6i+?îÅ%؇¡^?±oTÓß?zKpã½?šbŽsr"-? j€nÍ©?ªæy+ªBP?ì!j³D¢?¡ïw3Ti?™#"Ð6I?ŽsՎmbe?¹6+öXSä? OÌÜüÈ?ìYírçNò?¶GH¤[?#K®.@W'?={/wàá?½&hH?¶HC9&/4FGL J0912.5+1556?ï÷š«(@C#,¾¤ëÝÀ:™&dî—"À<uÄsa÷@!%³fm?ý§8ô=T?·—•á|Ý¿«¢%¯<4?ó$ہ›v@½íc›/ò?âúw_²íþ¿èSľ
'*¿Ó˜Í¡ˆü=¿ÝPô¤­¿èæló"
?àã"C÷¦•AGNbll3FGL J0912.7+1556RX J0912.5+1555?ïs‹¤TÒ?‡ó_1""•?bËtç.r³?``t‹päƒ?Žj_/?…Æí2•Sê?ïWSfDI?šAùsSt™?a\j1†?kU¿­þ.?›4ª琰?˜»¶ÓGi?íÚµìö D?"gn° íÓ?€v̯ñc?wÏ:Ú?ü?®TC}qÿu?'Xí¹g[?í3)Ó(?›v-Îûm¯?‰8½@p?ygž£á{Ñ?´wfç	e-?›-½Æ>ŽI4FGL J0912.9-2102¿È;…|¬#	@2|!ïAÀ9.qÊG·OÀ;à{.t‡'@ @É1aÌÏ?ý‹ÞÅó"¸?­ÐÂ¥¬wm?ŽÈfƒ4C?ဦÿÝo@Ÿ°É6¿ÜÛ@­ð¿åŠÉ>$(¿Ùeåvø…¿Ü=Ì4!¿âø?Â7È¿¹U@Ï(AGNbll3FGL J0912.9-2104MRC 0910-208?ï>ÂGĊl?‰d_?¥Š?YhOX‰?OùÁ
»˜Þ?––'}|Ô?ˆªÊÑra˜?ïxX¾H$ø?‹bC¹º?UdÄfT·?føðy7ð;?=L•i÷9?ˆ_'ó¯Ç_?ísë9'Ð?œð%ÓÄœ?ƒÙOߘT?xېΑæ ?±å|7~|	?š4õéè@?í^»¯ûBy?˜4]…?"÷ÎýP?m6f.vÒ?²åÝl‡?–¦Ð̳E4FGL J0913.3+8133?âíç•Gr@?ʝ@îÙÀ;qøòŅÀ<öŽhãï(@!¿ì÷åK?÷ìˆÚ.µ?Íßa$FE?ÅgY«m´?ûB=ú	F@Sx]3â±?ìäâ½ÏÙÈ?ì6«Ô.Á¿ÚÙ=—À|¿Úͬ;ç%?µ‡Kä/¿ÒÀ>ÉêDAGNbll1RXS J091324.6+813318?ïm—-5n>?‹˜[…õ¥?dÆY'$?aòïÖ»n?h®œZ§]?ˆŠ~D5ñ?ï¤?ªÀL™?†tօjÆy?@ÔS$Xm?[R z³Ú?…âЧY2?"ß:XH%?í|'ÌÑqs?œ‰ûR$P?lŒU¶"?dýd¼²?³7†ð략?›ô!+®òÐ?ïUZ¶¢þÛ?#'!Y?UTžË¯£?V·2u‰œ?"#á³io?€ˆž<Cò4FGL J0914.1-0202?êÃD''@>-inX£/À:è½±¦×À<[íâÇ
@Á_»ýF½@ûÜA´Ö6?Ã&¥]Œù¿§I#4{S?ä!7Ì¿a?þØ^€¾×A?ïù%P¡F¿ÙsûD¯\y¿ç™$(Ô4 ¿èyÚçÜs¿¤L߁°CÕ¿ïlìýļ]AGNbcu1RXS J091407.9-015949?íÃ2ÝZ?¨ˆš2Ù|?z8ò-Ò?rýԝ ו?°D"¹ò]?§ŸË$òuê?îїJ‡?zNÇé‡?ic4pý˜ó?yiÿ!Ôó?¡PX~U
?šçÎBç?ìõØAVµ?™Í²ªñú'?½ýäPx¦?ž
††ê?´™~;s;F?–WñhðºB?ínXÔø"Ñ?˜áŸ¨aï?z'§Ö¹™e?rê¹æɦ?²äÚÐ?è?˜h[Ó¡¬4FGL J0914.4+0249¿Þ4¼šÐ{X@@h&Üã›EÀ:æ*|«LJÀ<X˜џš@¦A¡µòÁ@Ìî?äž?Á!95«³x¿°ŸíË{?ðn"ü¡¦®@Ӈ[Ôg ?íòãâ"¿é.î•tpë¿êt»(_šš¿âMaa™Î¿×&IaÉ¿áÏïH²AGNfsrqPKS 0912+029?îŠGÀáƒw?œ:n§"9?urè5º€?l5yú?¤­&ëG'>?šà/~æ?ïI*Ê{¯?ƒ;$I?U>REZ'˜?_×o3ŽÜ?•ˆ•'Zâ+?iq'4Ñ?î%ÜPy't?æYDòã?w£Îþ´^ª?eµºCáéf?ª­Á–üó?·÷܌Vç?îÜqè'?Š•K†ìß=?gèK—[p£?[¦h°=ú+?¤£´(Ïê?‰4j—)É4FGL J0914.8+5846?ï¿RÆŒA@D§t¼j~úÀ;U^½ûx²À<ö›]¾÷ø@b#¨§?úåP׈èq?ÒÜù€4à?ÑÃa~ ?ÿҖÀ¡E`@':g?ï¢w÷ˆ¿Ø÷£ei}¿á"i·S¾Ä¿Úa'¼]hç¿ÞÁ[)œ\¿ïÿíöé	AGNbll3FGL J0915.0+5844SDSS J091451.54+584438.1?ïÍ¡Y?oÐ|¢p-?T ohï?K (Ì>»ò?tQûÖU0?k«}ÒÓhÕ?ï5ë:5õö?'Fü*I»°?]K¢–î?hp¥¯=ÕÝ?—mޘÒX?r|ÑF?í—
‡ßË?•GF—Î7?ŒŸÄ[ç'?~D×D^S?¯gfkN9o?'ÁiÚpü—?î«ëÚJ^Æ?†ÐÝ	!†?wåؒ?h?jnÁ+m?¢DŸ€GË·?"Ù-Œ?44FGL J0915.4-3027?î›é¾êG@)g¢xåÅÀ9ÿϾï"xÀ<49O¬æ}@
¾ýVW{@º–ic?¿Èûà3÷?ÄŸ€
s@Ûc[+J@ª¾MØü¿à–/¢!M¿ÌqÇXÅʿ㚾È'Kž¿á™!¶3-¿çY$Hµ¿ïýü_Œ'…AGNbcuPMN J0915-3030?ï¤TË¡ŠÆ?+T	ō?iÕ½ïds¿?côÑ°.²?€u]›Ä1h?}õ´gÙay?ï3·±þ":?˜4ÇÚ澈?egÁü<?s§ß â]?–ܐ5\?–*©
S§Ù?îèô‡M?Ž|uÈíô?€1A«T?u°TM0å?¢Ír@L¶@?‰Š2'|W›?îCåšð¤?"›P5¹­8?‹pߺÕù?o¯«ªjL¬?¤òi·­€$?°þ…{÷n4FGL J0915.9+2933¿ÓxõŠ0E@Ey…H©¼ýÀ8¥	pÂ
À;-M@$³@áòNço?üN™´?¥à¿Ôu?´FƒÇö#]@#¿µ'@	kèhߒw¿Û·‰lü¿×üè]÷×è¿ÚnYåN£Ò¿Ù‡'›x–ë¿âcÆ®¥šY¿á—ÙÛ©¢AGNbll3FGL J0915.8+2933Ton 0396?ïxÌn²?ŒÑµ` ?Xö>Wb{?S#¸§®e_?ŽÙEsЎ?Œ	 @?îk$GRô?¦ƪ´K™?|ÝÁ"'ó?‡&:º§?¥²góŽR?£xbØCÒ?î,V	œ1?¹¤ùÙQ?)‰nÑò?Š#Ø		#0?¥p= cèv?–Æeuv.Ó?ì%6|óm~?¢qÍ·è½ð?¾FЅ+ò?zk[5–¥!?º¦ºdCI?¢÷ó³ÑŽ|4FGL J0916.7+3856¿rõqSÐÈ@FؤTÞÀ9ÇÑq6À<Z«m×sð@}Š6OGf@ ôQvY?¶<Œß].k?»éß,Já¦@#³é¦ø'@ş\§ê?ïøª*s¿áŠ2¾™-c¿åV«¾	e"¿çøä¸{Üð¿èÛނ׶5¿Þú@MxAGNfsrq3FGL J0916.3+38574C +38.28?ïBy8ü/:?"x0ˋ=ú?cŠ[ń?X;:AA_{?•OǕ /?'¢'"yG?ï|`uôŠj?Œ`¿fÐc)?QáϦ¯ë?bqWš@²
?Ž«¨ŽïJ?Š"£'óc"?î÷«ópU?†¬.dÜçÔ?r&K¶,é=?`òŸÿâ?œ€î¤a&?"B–ÒR‰?ï"0CX×?rÅÅÏÏ;?y€{¢M³??cgi}Öò?'>vñ?kÎ÷Uj¦4FGL J0916.7+5238?¢Ýy¢–3@EƒÖ¶Zš€À;96À<éaB:73@ ©³"Q]ì?ûbU)þK?ÈvnfÔ?Àž«;ØsI?ùŠý¤/ö@›‰¿ÜÏN¿â±/bn4;?ï[$éÄT?¶œ µÍ¢¿ÝåœFó¿Ú/¼TS¿è®ÏÁsÓ6AGNbllRX J0916.8+5238?ïn®'Â÷J?ƒrVjEӓ?eAÿKØì?p}Û§/\w?Û|7@?€CNx–?ï€Qö(?‹Až¶')Ø?IýÖW²ÄD?W@bKTY?Ž€ý‰µ?‰Ð"$¯®?îÕïWá?
~|ÊÒ­?tt…Y õ¦?aVA_\"?«"_MÐ?ŽßÖºÆH?îð£ª#6?ƒq½l+?y°ÄâBT&?lÎpÿڋ2?›m2++?€ûEâFå4FGL J0917.1-2131?èoè+‰+ô@2ëÊÙ­…àÀ:¿ÒóW{À<WMÒ@ê{áLá…@ÊA¤åþ?Àoºx¿ºc%¿,P@?üuuGª¹}@@Ÿ¼}¿ï»…|¬#	?ëÈóĈZ­¿åfl{S]u¿æ¼QքܿÕsϛY–¿á‹½m´8AGNfsrqPKS 0915-213?ï3ÜêY€{?£‹™ìƒZ?{v@Œåè¢?€_8šì?'¦Ò'–vb?¢­Àq¨?ï WÆ]Ø`?Š>Qéøl?SC(-1B6?sº‰Íd–?…©b㿦?†«€>íèA?í³ôáƒî?•¯×'B?Š"ú6#€?ƒ'ÊOÛ¹™?®?"$cø6?'‹ëë]'?ïftÔ£˜\?€qfNziš?`_«°†ãÓ?]E+ýàH?'%oõ|?~hÁb€ËV4FGL J0917.3-0342¿ì»"n›Ë@=æ»frû À;.Ɗ"lYÀ<˜-שŸ¡@!ºÏ ;Ê1?ü»-Çüƒ?Æ˛ÊKh3¿•ò†Hõ?Ñ%'×µ^?ÿCûàa¿ïûjÚim'?îƒÓ"g*²¿×Êühñ¿â×ßð•ÿ±¿Î-›™¤{¿Ô￀ˆühAGNbll3FGL J0917.3-0344NVSS J091714-034315?‡Ã?€¢p r#'?K»òÖѬ?C*Ìå¬N
?Š¼]üA¢;?€3=(i_?ï3ö?St?"æÑlÔ
œ?XMaG¦[?f><IJÔ?—ü`{–ß?'¤½\8!?íìÖ`zEˆ?¯"Ìꞹ?ybpFòÁÚ?jÿ›èO©I?®Kï}OB?Z¼P0×?ìtÿ_àvZ?°°´0¹€?xFST§™¹?pÃÅn;"?ºÓŸË±Ó'?žù֞¥4FGL J0918.9-0625?æ|'­l4\@<©ÏF#ÐÀÀ;(ZµX<À<§ƒ]2L@ÅÐon¢Ë@Êô¯ú?ÏâXûå?Ó'{ˆŒ?ûûCµBm@ó^'í/Ä?ïã¯1±Rô¿Òþ"Õ½6W¿âòžM]€å¿èú'7¥ˆ»¿ÜõÿRÛð¿ã¢"Ÿg8ôAGNbcuPMN J0918-0628?í1G;C?§ÙJÙ%vÜ?…9?£9Dë?~òàîA¨?³Îž1|Rè?¦éë
þ›?îPô͊?§í0@r?…˜Q{¬?•æŽ2Æ?¨Ôë9/ˆƒ? µÈQ©7Q?ëënTð? ‹CJ?¢pw/û??Žï1<[øW?·oâT
Zç?—-ÒÀhi?ísFw@‹9?"÷VQiÓô?Tlu9?Ú£L®"Û?°e7*úÈß?"Ÿ¥:N2V4FGL J0919.3-2202?ïæpOt…@2ù€ä–íîÀ;rûbÓÀ<²'{J@!VhÏÍ2M?û‡"7Üæ?Ô"D¾Â?ÂÊ·H×	g?íds²C­@Á5±]†?ëޖxÓ¿ïynìFå˜?à»ÙÊâ¿å5ü;Oa¿Âák)¿é$ô^NAGNbcu3FGL J0919.5-22001RXS J091926.5-220052?ïIW¶U ?'Xó$
ö:?U]¦?RuåH›¤Â?•"m¸OzV?'Ú/ê"
@?íê¥BÀ?µ ªÞ4Mx?lÆ"9Ô?|]´TOó?°üzQNÀ3?µA7ÅG?Ø?í[D-¢ ?˜°âQ­t?x'O3}¤Ü?hënï?³œÉŸ·h­?–à~Ì¡B?í5õŠï¼?œ"
©¥€ã?T'ä9Ž?R,Yœ¦ÑL?³´Œñ0?œ†'éyÆ4FGL J0920.3-0443¿àº…Côª@=ñ|^ö/À;+×õûÀ<W$ü8Ë#@˜"vm@wŸ©~+?Ë\(	‰k¤?´€ÊjÇÊ?äIRÄÈòM@	 ]Ötì?ïòãízÂ>¿èHyìU(Q¿èjd!舿ê1HKÿ¿á½¼>	P¿ïùœÙ¿úVAGNbcuTXS 0917-044?ïÜoJE™L?n¢4&Ê8R?=·Ä#¡W±?7	§@:?oÙ½5ò‰\?lêY`1±¡?ï~¤û??™&NÂqíz?d±'®øÛ?shÚðx0Ô?š:ðI?•æ|EÀº‡?Ž 
?Š&§t@î?r]êÛÈ?flÏò±—?£`ÆRAÔ?ˆ"
zêš^?î¦vÐc?‡`Èþ*+Å?fñ¾%¥R?Vó;ӎØÃ?¤)ƒ7t{?‡¬Pi4FGL J0920.9+4441?ï*Åë 
Ö@Fgb(EÀ7ÉÑæèÀ;8àò¿@Ì8¢2ðB@#szK¹? Í&Ü/7È?Ár3y)6°@&…ô¡'-@®uµŽÂ¦¿œæAE£*ð¿Þ%[Z™ª¿å&=·³à¿æ°üÂ]޿ꨢ ÿ>¿íêi*fAGNfsrq3FGL J0920.9+4442S4 0917+44?îÏq²gO?žeiÏ ·Ì?‹¡ñYðH?‹O#úîŠ?™½ºÏÃ?—$è×MHÍ?î®.‡x¼?¨üPšžu?y}m,â)?‹£¬B½™?¡íwzØgð?¥g.w/˜:?ìùóvy?¤É¾‹ç֕?¥¶ýjŽî?šfçKJÛ\?ª©ÑŽy…?œÇ­®²p?[+Üá?š‡}—¸?wäôõ³?q¶}nV?¢"ýÊã"3?˜gŒ)ìÑ94FGL J0920.9-2256?à(:­ê£;@2¥…7âÅ]À:ÙjÿR[À<€[wõÚã@!$ï$©Á?öâñLO?Ն¥ 5"?Ö¬ƒP?ÿýf¤S1?÷°o̖œ¿æx="ßEu¿àNÏÜKÅÑ¿ÎK*
j'¿»Õ9'ØŒô¿àš¥½ê0á¿àõ–AGNbll3FGL J0921.0-2258NVSS J092057-225721?í`=¿nL?¨–·t©Žè?tˆ…×ã)ª?lž€ôPv?³µ‰§»?¨ÆCjù'?íw4‡ß´S?®Òg_?‹û¯8°ò?•äÀÒª?°ÆåÙìYÏ?«DøŸ?ëy×þ¤­?¥iÓ¡ä.á?˜V³
ù¼?ˆý´ØRhŽ?¾"G\PÏ?¢mwÞR'"?è+¢]˸?§töîs¯?àËà
ƒS?'Ò èlŠ?Íu°¸‡øí?¦ƒvÌóðR4FGL J0921.6+6216?Ƽt^´k@Dᆘ5À8LPíX^À;ê"lXî¯@"ýð[GN@ÇìoíÏ?œMÜ#N[$?µFß•d¬@2è8ªk@¾j£Œâ|¿ÆÉ™;¥È¿áΪó^1¿ãÝ_~Ù¿å‹V	÷Ї¿èém¢ð¿ì,ÉVö†ÚAGNfsrq3FGL J0921.8+6215OK 630?ïx©ùŒÞµ?Š.$Vgn½?h'ô>OQ?t,IªM;×?‹±$>Ë?‡\Ò®?ï\$¥ÚΦ?š¿â4V>ˆ?W»7Ÿ¼Z?j`⼉Ñ?'ÿ·Òü/Š?šðN¨J,?ïH6@ïw¿?†´ùà*	R?uϳÀm
"?wÓRžåŸK?'…Jñõŀ?'ªäD¦ª¢?ïû±øô¤h?3vA	KÞ?"×N8Y]?Œ6´_?;炇N­?2ò«£P
4FGL J0921.7+2336¿ææŸçÖ,@ElÍJ¡À:<—FÙeÀ<xÀŽÐè»@¶õ¼/E¾@y@þÍÐÙ?»Ø5õ…S?`¢1Áä©r@K®+÷Տ¿ã­ÕÀ­¿æÝݖH¬A¿àîŸéiæ¿Ú$;ɄĿéÔÞF-⿸«äIìPAGNbll2FGL J0921.9+2335NVSS J092145+233548?ïÄJJg?u°	¹ýVÑ?T%q•™?P§‡ÞS6£?xѳõh–?rՊ¯£.?ï–~ÖÙòM?ŒBžS´¢j?B]lw*@?VÊ"@k×?‰:s'Ë®?‹ÖWÜ`Š?îãójº?Šx	vtï›?sv,åj…<?rXöXL´ð?ž¤odúö?…ϬK¯üÕ?ïs=‰˜€?u[x&?c­ÈÃvûB?QDCbÚ­?ŽE+Œü!?s
ø.w4FGL J0922.4-0528?Þ%iÏ°
@=푼U†DÀ9õ×CHT-À<WBXj$a@í™IÁÉ@[A9†3‹?º½ó×þ"?Áû¿i!@¿l\I¬ò@I1!`"?ïú=³¿µ?±'Ò*.Ò¦¿á7€—9î¿äW~Áüå¿Þ:Ó²¿êc'@ßÄ AGNfsrq3FGL J0922.4-0529TXS 0919-052?î*Ö#!j	?Û&Qî»?'ãЩü²R?µÊÜ¥?£àµxëM?"à=§sf?³—Û'? ‰è*™pJ?'+ùi§?‡ÿ/"Ù?¢½¹ÿƒó-?šø£<1¤?ì'aq4³é? Rß7vÀL?˜Ü0‰ø?Š·ô!þ8|?µ=Í*7â¡?˜µ8åÓ?ìä´A?—šØÛjê•?«!=ã'iÀ?'ˆuÚ‹?²`@ø•>»?LáŠÎ9 4FGL J0922.6+4454?ëDG¤üœ@F‹«ud0+À9»ˆpSOÀ;;èné§@lY­ñ?s@µyyh¡ª?µºÎaf;7¿·B~"%¥@¨š¾\ǁ@zxnљæ¿âEà_PÈ¿ëÕ®Þ]¿æ4ò»sÞõ¿ã'
?ىʿïò5ýgõ2?îÈïÈzWµAGNbcuNVSS J092235+445749?ïãJUÀI&?pÄîÉAc?]³XÊäÁ?cWØöB?[·ûÿ¢Îä?eê—Ozü?îÉæØÙ"?¬ã4MtÕ?t6='ªà[?"l!ÿWð-? ÚÊÍzzÁ?¨""ŽN?숌ÇHAR?¤[7Åu?–fë]?QÛ-Ô_:?¶6À
没?¡Dm-¿ÂI?ì;ZË£?ªÂÕÛð	×?vú#,€™?rXöM¬?º–'ößá¦?ªYÔÎx>ß4FGL J0922.6+0434?±~_Må³@A»´_½ŒÀ9Òþ?5 À<7•óëï@šÙlmf‹@͉ößÆ?°&Ëƽi-? 	ߧÅ×:?ëG©Â†¢Ç@=zœ©C†¿ 'Ѐ>T¿ßz}	@¢¿ç.,Ε#é¿èëaŠR¿ç»š?±Æ·¿ÖŽƒ»áÂþAGNbcu2FGL J0922.7+0435GB6 J0922+0433?ïØàÃÛ¼?oXÁÄ6"s?Aô`ÞÄÊÄ?5µŒ®-s?qQ_¹ˆ?n$1
ÿ+?ï»à_O¥­?~ŒÕ¨VÙ/?6&´âú?N÷©$<s?€V²…ÜÌ?}÷7œÙM?ï½•]öæ?ƒ¹Ÿpv^ò?o1Ÿ*½~ü?[—ÛÞi¹.?š'nés|?'7ôy?ïòã²-Cf?D¤¿—¨ºg?3kžw'>?"rÅ'—"?U]´·«?BéěvÏU4FGL J0922.7-3959?¾>˜×|Ô@ƋýϤÀ9sÒì¡~jÀ;ݸçì
@}"£˜öÜ@ƒˆ›D"…?¶hÛ¡%ÿï?¾¿Ïä.hH@Aƒùdo@Eìs±(¿Øæ4"E¿æWãa
áë¿éZ~›çQ³¿ã'ÞÑ·¿ì
ÓØZ¿ïÿƒmÞ)ìAGNfsrq3FGL J0922.8-3959PKS 0920-39?ï½ ƒ,v?t~nþ¹¹v?b*`[f¹?lì"lõàD?xZËý¼»?l¥¹³ÆfÏ?ïCòlÝéO?¢ÏVEK?BÔϽ=©=?b`1UƒÒ?–ëæXè·?¡ð¹:ß»ù?îP­4pŠ?Ž%÷ɘ?ƒ"ÆYø?uBh¾¼ãP?¦Ær°s?‰Ó9éö
·?ïÏÞrúÛ?b>}û'¾?J¼A<e?;Vˆ¡oN®?t¹4zÐ
Õ?`ÄCB§4FGL J0923.5+3852¿ÃvŸ»éòð@F½inX£/À9ÛýåsŒÀÀ<"æu@V¢NÉç•@ß09ƒ¯M?¹¡®æÝÅ?ˁR:Šj}@
¸e6»~@ÕÅCìi¿ÙÑãl'¤¿åZ:8
3¿è›!>>)0¿ê'?_†¶¿ïÿöût€¿Ênà]xV(AGNbcu3FGL J0923.1+3853B2 0920+39?ïÁ'
6·N?}øá;Óª¨?x/œNzÔ?yGCh¬·?\u5WxÏ?]÷,Nú‰X?îüå¼Nş?¥ož7ß?f߬Ý҉?€Bsˤ-?‡RچQò?£—@Œ+¨?헋Ȭ?›Íro«K©? €(@ªÙÕ?'cƒ²K•ê?¦%ÂÊda?èß)D[õ?ï7L¥
-ù?MCª38?'3²0?mÁ˜€qŸO?¢Äá(Å?yÎ×útx4FGL J0923.5+4125¿Õ×ã%\d@F¼	ԕ+À9"+¸ënÀ<i3—Ý÷@QÞc£"@xAàu >?®<ÃÇ
–?²ºýíV/7@÷×ûÕ@
òÍtg†¿ËæJâ§T˜¿ÝOÍ¿å×6èÊYU¿äe8Ó¥"¿æÿe I¿ìÃßâSGAGNfsrq3FGL J0923.3+4127B3 0920+416?ï(ÐÏ?'ÃòÇå*.?[Þ¢£¾
?Q½ýòÊv=?™KøÒJ7?'[ÉÞá…ô?ï€?}`?™ýëžmK?g€6ÏV?y8ë¼YG^?šlY¨	zH?–Ðc¬^=‡?ï&©&<ь?'=¼mÝ$?mçÀ@û?[ÓJ€c÷?—mç€]ÎW?€e™Þ–Ä?ï.àMï?€ó>MTí?ŒÒ˜
f–h?v†d£t÷h?‡uT²S-–?qß_*4c|4FGL J0924.0+2816¿âÈFL.p›@F7ë¯#dÀ9î—ÁREGÀ<zãv\}¯@]ðáy@.þOü—–?¯‰N?J¿¦&ú?̞ª?ñlj	ÿ]@A<%J<d?îŽÃ|Áò¿äÒ8\gà¿èÐ"uE&¿à×J4¸¿ç>àæ_E
¿ä+"XÖ[AGNfsrq3FGL J0924.0+2816B2 0920+28?ïäzÄ´í?k¤èÄ×í?B5^Êpü?@Ý4›|$+?f÷×s`Wp?h‹…¯Qu"?ïé(ñ^?ˆ%
7?AxTºX
™?R)L!*ß?‡n:j'È?‡(¤Î¯JØ?ï,c{Q"'?£—¡žS?hú¹?hÏ?WC!7/?—T9mî"?|ÓGÒ¹(?ïì•9\u?L¡›Wqç?FýE}s5?5QÃH?\x3]ô?G†"Q<yP4FGL J0924.0+0534?éaÍ.5aP@B#Bþ'Q~À:ô'ÛçÀ<ˆë"²'@ ,üÉÚ¨@â…Ãù¿t?©Ú—O¿¨é#šŽâ?ç·4Ã@	!'Ë?ïœd…D¿é᦮U¿ä³ñTk'¿àÏ;<1¿Ñ[=E@¿áãXàÿÇAGNbll3FGL J0924.2+0534RBS 0771?îÊ+åŠ1´?š$¥"Å`?j#£Q—
D?amç4~R?¡»rCt"?™$Üa!Õ?ï-ÛLý#?•Kê?r{Â?^þl°!Jï?r÷–<¡Lº?˜T¯•Zæ÷?"®½[+©?íæz4ýŒ?"jÞ®>Ž*?uJë¦]è¬?b$<`vk?®îÿ;bz%?'T™q]à?íЯ׭Ð?"w*è€c?w`ÅtäJ4?k"=d—?°tëIDÚ?'øqD©Š4FGL J0925.7+5959¿äKÃè%ã@E sÞ-èÀ;-Ówá¹À<àì^b‹æ@ ¤|Ö?þb7G"ê?Å1®ù¨"?¨ËPö½Œ?ä8j¤ @"Zî?ïòÆ@Á'/¿Ö–"'I¿¿á´b\Ô¿á[þ˜÷³*¿ÔOd!ȿۏ²tƒàAGNbll3FGL J0925.6+5959NVSS J092542+595812?îä'Z¿µ`?•ù¡OšÞ?T'ûŸîiœ?Fºßè¶E/?¡Zw6©?•.â'+?ïoöVùä?‡R=7S?Cšƒe'_?Nñۆ1g?'dhù÷Ò(?†Ãö,&'»?íè´bÈqY?'ø#ÑLÚ?t'ù܍?b߅Ë?®ñç"=jZ?'+nêšÊÖ?ï
Ww€‡º?€L¦ò#ö?mî*®t?`=šPˆ?š—Kº+Ú9?€OëÆ/$4FGL J0925.7+3126?ï/{BÁq@F­"àÀ:…¥>éIÛÀ<«ªïê@VÿYfú@ƒ¸¡œZ?½‹.`ªS•?™€È½H X?ÚæÞP­Â@'4ð!»'¿ÒJÎZk†a¿àÜ.1k³¿ä±3¼Åï¿ØÞd$í ¿çáӟyØ^¿äWŸ#FVAGNbll3FGL J0925.7+3129B2 0922+31B?ï¾Êù™?s©æ(4?SžOœ¦è'?Iï«´¬¦F?{²ï‹Žy?r	Þ†;?ï˜0QÅ
?‡Å|§Ÿ"3?Ic'l?Z¶£kŠ?ˆ]»>ŽZ~?…÷Ü$¿ŠY?îmęêq?@Cþê?w…€}=­?cZ{&Éá?¦B¥±IF—?ŠN†c©?ï‹Éۘç?o6¤¾ST"?sVcˆ•ša?\^á3Á`e?ƒbWU{Nö?hÑ!ǞŨ4FGL J0926.4+5412?àæ>w
@F	š¿3‡À;wžYóÀ<؂ ×@ 6PiNù?ýÙ¤K¤CA?øh;ӕ¿?²ÛóÚ­¶?ðÁàŨ]@㉠þé?åë¡òYN?×_×Ár{ž¿Û·¤F›ÅÄ¿ÞqIþ7(¿ã ®Ì0ś¿ÕDzãíAGNbll3FGL J0926.3+5409NVSS J092638+541126?ïžQ¶çyŽ?{
óuí?PvAf€S#?APB-«×‹?†\ÊQ'9?zG­»
•¶?ïó­A%?‡ÈU%A?G–wnË?S…Yfâ£5?Š‰¸¤¨ÉŸ?†ší©©ðá?î–[Q3µs?ˆø"?óôz?oóĽéQ´?Zwè"ê+c?¤› æ»?‡A'åv?ï&þj?z>øh¦—7?xå*Žl_K?c‡wfQ?•՛צo?xՍ}u&4FGL J0927.2+2454¿ëøëâøÄ^@F2wpyåŸÀ;0èÈ«ÕÜÀ<½{µƒ@*Wú½ËÓ@ ߛÜiù?ÑÁ‰7Kƨ?Æ#G'Ëvá?ó6¯Ž)ú?ù†ßúüá¿ïØgHðŠ?ïÿ¯"AôA¿åŽvàÜú¿ÐèkÄt8·¿ïûÆ«±Ê¿ãì5YAGNbcuMG2 J092720+2456?ï[*žk_N?O²Óèû?iØÓªv?d¢'?'z'1àá?ŽizŒ5(^?î@—i?©á"A¾?‡:$:~á›?"¾D—:?¨íu¡6Ñ?¤!™§yñ?ì]ÿdƤ? yÿq?™rÐ.Yàj?‰ƒàtrZ?¶³PÎ4gm?šY™œøps?ìÃy-}m/?žî1͗lD?¦ÈkÂ?•Ì4òÆ#=?¬ÿë½k?' ÿòڗ@4FGL J0928.1-2035?í»¡ÅsMf@5x¦—®ÞÀ9þç×NlÀ<c$—Žý^@ÐOo õ@Šúšeq?¸pÀ\Àº?¿å©érö@Ò}{Uá´@ºÉ,YOR?ïªFà!q¿æöÏՕɿçAȌÌ+½¿ç€Ú")=¿êï$°¹pÏ¿Ò/)"ä¤AGNfsrq3FGL J0927.9-2037PKS 0925-203?ïÏ£ëÕ¦›?uj<",K?RÅtÀ.´ý?NfÚß
ç?s|¬å!?sݞú
E?ïºnG%Ûi??žç:?F™\†i‹?^ϓå™ó?õ°ÜEg?~»–£ì¦?îæTuT›?‰²±åøªÔ?vx[û¯y?nê¹ÀŒqý?—fiŽ&?†¸.1¤õv?ï×{(ӗ?]OWHÏm?UL žî=?B¹Qí7µ?mއ²\ñ®?Y¦I÷·<4FGL J0928.2-3048¿ÕH΀V&¨@,éáŸÂ¨‡À:Rۗjë0À<(<˜6Ã@,LÖGtß@ùúÊ9?ÁÉõA‹¾?¹Q"º•?ö]‡ëlm@¿!"µ?à7Åü-ã¿å—Ae%Ç¿æü¥Øl=¿é6sXg¿ßc¼ÑG¿ïø*ÿ2$ÀAGNbcuPKS 0926-306?îضŒåì—?£J%É?f9l+¶?`hËnþ?¡nå5?¢¯[ÖûSy?îÉ*¼[º?¢;ËD2?cÖ|ÿaó?rÍ­3oE:?¢/ìjN@?¡j÷3t?îwÓɅÁ˜?¾zð˜T?y©Ý¢…?m³Õgê}?¥Q,%?Œ0MK¿?îS)žRÑ
?†®kÐà—?w‹shæcU?cµ1Þpi?§Û÷­¶"Þ?…*7»¹D­4FGL J0928.4-0415?ÖzFÀ%A@?Ü_õHíÀ:"a‹5RÈÀ<oÙzZ91@vœ#·•-@Õ;f›Ö?Æ˃ ±P?º8öLÖó?ñÐD¡À›@	¥ŽÎºb½?ï¦pý™s¿ä2î4%¡z¿çe`!Ràø¿æc¤FÞâ¿ïÿø]ˆò?ê/†€b;	AGNbcuPKS B0926-039?ï¯ò¨Wð?žÌúB?\î¬Mö‹?€»²ûÄá?€ ­Ô E?–ªïúõëú?ïJõÍ|;"?"! 7ª^f?`Ë°²-¦?p¡Æ»À]?"‡ãbGÐ?'g6í¾6¤?îäìU+?†»anê%ô?s\î)ٝV?_ºµŽò%?¡Zzoy¡?"åB2.¹{?ïw_ǛìZ?u¥9N[?oÃJf&{?\lËÎJõ?Š7I†k`?rSs
´ï%4FGL J0928.5+4048?Þ7ŸdÅã‹@G7žYò»À:ÝҜ¦šÀ<Âc:aûž@²Pt·?ÿÆ.¢<Ö?ÇYü ¤ü?¹1ÀíE"2?òB¸ý/¹@ z~¡Eµ¿àå´àFý¿æžã…uö¿ãk®Œp¿Øåøƒã¥¿ářœô—í¿ïÿö$´ë/AGNbll3FGL J0928.5+40481RXS J092837.8+404858?ï³Í҉/-?x0m.â&j?P¥ÄÁҖ?LŒákÁ?€÷Ûeú?vp'ÌX[?ït"þ°˜Í?ŒŽë¿‰—?K·¹""òå?U¶`ª½Ðo?¢]P>?‹@Æùm?îdâà}Õe?Œ LžÅ½ù?r"6ݤ£?[?ºÃ:?§_K'5*?Š!–ï­?îçkey¯?€§Þ!÷@.?x¿õ6@G?cå3æº?cS|Ó?ч!Ö=4FGL J0928.7-3529?ãÍúR¹X@&p4 ½À:B ½å©=À<0d~.Ú@<gm!–~@ã`ݐio?»»žÕ(ø¿cD§"œi?¤£áÈÂ@ҐöÝÂh?ьPû"¿èKƒŒÚ¿â`c&¿à3Vn¡žK¿ç/Ë¿Üyh¿Ú/\#—^×AGNbll3FGL J0928.9-3530NVSS J092849-352947?í¶ðâòªó?§šËô¢é¨?kp)ºÎü?w'³ù‡´L?°
ã3N‡?¦ÎåsU?ìZ"
S?¿)ö0€/?gAtœËÄ(?tQ¶kê?¾Ù†7E?¿IPšÜ
P?ë¹4'£gQ?¢tÕé…*V?'xnȂ[´?}:€Tó~?½Ø?¸Ä.'? ¯ }^¦(?í[}¯|úF?Œ,mńD?Š%‹±ìÛ?oø 8ï{?±ßa !ð'?Š±tX¸f4FGL J0929.3+5014¿Ú‹þOj0@F¶™÷LÀ9Û~@w¿À<%êÅÜÃ@/Y­€@Ê%Ðt!?¥C'«¹µ?¢ó~½JM×?ûæ8^_
@ò{PÞë¿×R]šåÊ¿Ù^ØO·Î¿ãž"jc ¿á»ßá§z¿ßfÚ?&0–¿ënxÿQæAGNbll3FGL J0929.4+5013GB6 J0929+5013?ïˆ÷ŒQ
*?©w¥pð_€?S@ŽAnå?u£ì?¹0?‹Z+Gk?¦ßo)‹Ær?«À`3?‡$eS&ü?Hªª (?WÁbS&&?ŠÐ3åFHð?…÷Ùö›Ð?ï6xÜ?ïu?€˜9yM0?jìºð|ÃØ?a%çQ³ª?•ÓMòy
?~JxDE?ïÀµg?f#Ÿr:ñ?_SYÿ1?K±'ÍBÉ??wÐuïñìt?boÌ×I"4FGL J0929.3-2414¿î¦ÒîØn@3/ÃøôõÀ:úù€‰þÀ<›>»&²@~¥¢fr?ýTq÷" ´?Ô¿""Æ?Ùè'¯qr@  F\ä@b35e"?ï¬LŸ?ö»¿âåAã¥+¿Ôy;U@¤¿ã¸ÀÅ­¿åöü¿ïþöë"GùAGNbcuNVSS J092928-241632?îÚtÀŠ]9?™çpþÎ)?ˆƒÚ}lI¿?ó@¼!?˜oz¯þ3à?"²øC<2?ìÀðx??µ}_OÇ?šHy#?œãêMcŒ³?¸ç÷aVwû?²#×öåZ?뇛ä>_Û? !RÄ{Ì?¤†ž{Ö*
?ŽX-ùÓ<?¹Ñ !ì$?™ÎUáؑ?é2/ü¥Z
?£1ƒÁ0Æ?™ç_e¦Q¯?‡Vâ'•?ÇúT µÍ"?¡"Ì.š×4FGL J0929.6+4621¿îB0×cS·@G
 r~À;"Îa!ƒÀ<"«ùiä@þžl<>J@|ïÅYb?Õìé¢Æi?¿·ÿãz?ߘ¶…7·Ò?øSƒ""_?ï£XK±¿èo~¹Å¿ã?æŸÜ©º¿ëBµþ,Á¿ã.¨TGñ¿ïùm¿¡9AGNbcuSDSS J092922.75+462046.4?ï,VMs$×?"?ó¥Áîx?a˜¥©Ýc?cɵi'rY?˜B!œwie?"kUJ;/?ídª›Í?²;Zæ(§p?{•Z#ñ"?–L®H¯¸Š?³egÿâ«p?­"ÕÒ3W?í/tµ'ò?–#CZ¢n?'ìâ.æwŒ?…8É@f™Ï?²kΙʎ?'áG2qP¥?롯" ? >•Up
?"iSoB?ˆ3qe&ÆI?½'0i
$?žRU?ƒ×½4FGL J0930.3+8612?éùó¦LÒ¹@="%¿­)™À9h›WûQÀ<Eyõc¶@MßÇPa@–£E?¶J¸ o÷Š?¸y/ýÚÇó@u5'Ì÷@ˆ¿6Œ.!?·ö*NçD¿ß·RDËâ¿ã7³`<οá²+–†¿¢¿é?qdÇ)ö¿ãcBZ£‹AGNbll3FGL J0930.2+8612S5 0916+864?ïÍ×>
 €?oŒJÁøO]?WS"AAÞ?PlÜÊÍÛ?s?˜wŸoú?kÐ^9ʹÒ?ï–ÕG^<?"Ixûd?O+Ir2ô?]ù;éZ	½?ˆWùr͋?ð»EW!?ï#}Âaõ-?ùiÕrd™?q'£öÍ>á?k&iM8-'?—+Þ¶
?y͒™·ã?ï¨üdo¬B?m•ào¦,?lWEü•?V†ÎÈ#S<?}VM¥Ÿam?hA»ò3Ë4FGL J0930.5+4951?¦ËÄG/N@FØwîN&ÕÀ:ÌÉÀ¨ÒÀ<È±µR@!t1¹áb±?ýP2é?Áǧ‰qX]?ƒMŽF@?Åö€û=" @÷ŒV:_¿àÕ¿ðEwÙ¿ä<ôb=ú¿ãooŸ?‹¿ß2ù<†ª¿Ýnm[x Î?«Á^¥…iAGNbll3FGL J0930.0+49511ES 0927+500?ï¬ì¤ÿfB?z%›ûÛ'–?A£ä [î?3ûÃÜ$;ï?ƒª˜~ ¿^?y"…3h"ò?ïomG‹¾?‹YY¢Êz?IV±8¯ZK?U^üÍ0x?'GªmI
‡?Š,§ò4ýÝ?%ÿ:œ?‰TÞ¸·
T?hÚ©N/‡?R‹!•._6?¥h")e?ˆe¸ß­?îD•ÙX2¤?'zÙàvŒ?h†óéÒ?^Uošws?ª-ÐÒ
—?'Êã›s4FGL J0930.5+5132¿ç¼j-_""@FªJ¾j3{À;¿°ä8úÀ=u=™¾ƒ@ D߀®'"?ü¶¦4²4?ҒߪJ?Ïv³»ƒÏ-?ûtÓçsA@@¶©
оt¿ßÓ^Kå± ¿ïÿ\‹/ô?ïüSme^)¿ã;§««¿áÓÌ/îÛ¿ïÿþó…õAGNbll3FGL J0930.7+5133NVSS J093033+513216?îÚàím?§_lx0'Ï?]"O¨'?aâ<—ò?¡hÞ«íö—?§
È4P¤?îÂ`U$@æ?¤*#CZB?h7
ZÞ²€?w!<t­zE?¢VŠn?¢"VMà%?ìµðZç?Ÿ2²vø«Á?Í,9'sÊ?'–ñIÀhQ?¶–Ù¾ÙU?\†™¡[?îvÈîôg?"G_
HcÉ?h0Vš?hÅ8'7áŽ?§>V?¬?'‰C'ZZ4FGL J0930.7+3502?ßåë¤Ò@G`ÉÀ¨ÒÀ;0f('ðÀ<ܾ•Òd¼@ÜY·Vmö@+À nŸñ?É?æPl?­HPÑ©«`?ã"cßùOb@î¿æµ?ïê"Q€ü?·ÌZ ²Òü¿æòƒàÊ°"¿Ð]ãŸ''¿éÔ+{¯¿ïøÿ?æŸÝAGNbllB2 0927+35?îæêX§IX?˜ØkصÏ?m×É~K?e$J^Ä
6?Ÿ€Ùñç­?—÷f™y'?ïBGtö16?'Á
¹!1Ó?^Ãòí,'"?hñ…©»?•ÊÒ2g?áÁQ.?ízE€'Û6?•×¦]·ô?‰¨v|"?wí¦ÅkúÐ?°øÅ,ia?'ì;Nc¶'?în=ŒúHl?Šb¹?Z?–e"}€·Ñ?€¿Œc–=Z?›Òºã6:…?€×2â.µ4FGL J0930.9-1015?¢DáLyî@<µ?á—_-À:Z'¹hÀ<vö=Ÿ@æF×)òî@WUÿæՍ?¿]ç;ãÛÝ?´zr!…‹Æ?ñ+!Z³@ê$O?®?ïÿÕ%t.¿ÝÜxüÁE¿äŸNyà–®¿édŸ;ïð¿ááHtEL¿ïÛþ~ÀAGNbcuTXS 0928-099?ï°ÚÿB$?¬3^ÐEÖ?P$ úÖÖ?E~ë:mŒ?Ä¼"›é?§çæiV¸,?ï·÷<Ê`?RV¼ýñ?=zlö?RÉ®°º¡Š?]m~ß.?€*m«]Ã?ïE¥@?"Šï?A"?p@A™†u'?`|¤»
Ç?›gLûúÊ?'©J3(Î?ïÂ]¼RQi?apüÙØ?V'E1?E'"¬v.'?y1ZLóz?_¥i‹³4FGL J0930.9+0033?çn~ù¸Æ¹@AŽ'bEoÀ9›õœÏ®ÿÀ<G^ñýÞ¾@L°·mj@Ƭ!\?µKÌ ñÁh?Áö*¿@ƐšíV°@ÿ÷ªÖ¿ÉjW·¡íP¿åþŸ­¯Ñ¿é­'©èò¿ë0߁w^¿ïÿØþ3w&¿ïØAªÅ;AGNfsrqPKS 0928+008?ïÔl®(M?pí5Iÿ?e .'6Ó?kÎ4ޛ¯?f±ÍF{q?_¾Î	ˆ?í_ËdÄ"õ?¶?¨Lwú?™êÖâÓ¤?¨ÞŸœ˜Šš?­
ÞB±fñ?«&>¯\µ?îïñçˆØ?ˆ"ó5©–?}nŸQÙôv?xåÇ)<'½?š¦&n˜h?'êo¯š?í¯¿5?šŒ®¤|?ªYŽ]²FÀ?—͈>©?•Tó÷€Ž?~Z "DÞ4FGL J0931.2-8533¿ç_Չù'QÀ8:dž;îÄÀ9ÏÝ;¯ÙwÀ<H~@WZ¶"áÒ@6Øôù;Á?´4T_AÉ?™òĒZz?ã[é4â`@Û3¡íûñ?ïðDÁPï¿áŽÉý³ø¿é•lä.é"¿âÒ5!Iü£¿ê';ÿŠ;¿ïÿÔ@ßn:AGNbcuPKS 0936-853?ïç?A•
?[ÜOÏ%Ò±?Fì¼F§•c?;íÍ"ù¡ï?cYN'?X"¿ß®Ö?ïÈ/YY¥3?2·ùÚ,?(L¯7¼Ò?:°9ùlÅÊ?{%íÚó¨K?€«ó:º¾.?ï&ŽÄîFä?ËBVú(?o9ƒ¶}š?`'0î?—GÑÀSÕ?}B†à["³?ï§;foË?mØú ™Ç?\?f´E|?HóŸL¾
?'©9¶í"Þ?k|ü¡ó4FGL J0931.9+6737?èÒ2"®@Cåwž™À9õ*8¸®2À<Œ
¨y0@¦Pç}@ïw݇/?²õçMVŸõ?¦ã,Š¢…Ñ?óŸÁ?/Á@
¡–‰ÄºZ?ïÿ·ÀÌ
Š¿â¿a!-!¿å1ß«Ì¢¿âß5…¿älɌ¦l¿ïmŸ`=AGNrdg3FGL J0931.8+6739NGC 2892?ïÀ_XAèá?|ÓsH?ñ?FÝa{?ACfŠîú?|ô°[m?{"`ç+Ê?Â;ªs?"ZÚnSS?F£ö1 …?X¤6rE~S?…óP
û[?'ÜX&o¾E?ï0ét®"?€–´†Â,ž?iÂ="H?_'•ˆ0Ë?–ª–Ç?~Dbÿb?ï®KÅçˆ?hè¬õxs?qT¼("?YX*#à?w†n`ä!?c—h)Žé4FGL J0932.6+5306?ï¥væ)@F ÇŸfb5À9¡®×€*À<‹íóŽ¶@b9®øP‰@/ÜÌõ?¯S¾Ãõ¶?µBJ¨DØ!@Â;C¢ìÿ@†Èg¸K?áÍaýËó3¿ãÑG»€t/¿æd2Dꁿ炞«QR¿è7·6¿ãÐ9h×YïAGNfsrqS4 0929+53?ïBÿ*³?ÀBPL8?<¬[§ï¬?5×VB:=?—?¡i:ð?ÀCXEQN?ï'l%?‡h•WBF?CCT2Ù¬?YúŠpÝØ?‡'EáÉ'?†|Q`"M?ï»´.ͺ?"óh†ƒÏ?mµl'só?_ Ç©ËÙ?™QÛç÷ÔÚ?ƒy9y«ê?ïúë'®?5|ñޜì?-2…Š…|? –JbiîÝ?;IdÏ¥P2?1Ë®+Hû44FGL J0932.7+1041¿éBe¶ú8Ò@DIÞ½çÀ:ñŽd²1@À<ŸN"
@ /¤¨ìGç?ûüÇÓ¦Ü?Ì" 3§!?жIÿj.@S¥Ýt»@GmÑi¿Œ?ã[}i¸*~¿é˜¤ Üš?ÐÓۉÓÿ¿ÍøNñ¿âÝø©Êi¿ïÿ£^ilÖAGNbllNVSS J093239+104231?îð«ëiç?—œÚ®î?t½òU¤Š?j^ãGXõ?œÏmí) ¥?•¿€'Jñ…?î•Ôob1?œ¯ëW‹Ê?sôJÿý\P?{ê¬Ü<p0?¤1Y
1ƒ?™/ÐÕtM7?í8"›Eª?—¨ÛsD?Šhxbþº0?|D™3×`ò?²îÐfÅûq?"pák?ë_0Ñð^Î?žýÉDRµa?'%G<ƒZˆ?€	f®¨£º?À>"Ю}? qª^#4FGL J0933.5-5240?âM'>÷ü¿åÇòÝ؍ËÀ:Ͼï"xÀ;È$g¾U;@!B<¨§Ôp?û´ò»sÞõ?Îß$}¸½v?ÑhEƒíµÑ@½ÞÎW@U›ÛhF?ïeû7Cc¿é MÈ௿ÜÒýhv¿Ù6ªK˜"Ç¿Úó­¡¹M¿¿çÓșaeAGNbcuPMN J0933-5240?Ç1VCIºù?¸³îNˆ'?‡´|Íé;n?'¿
HVŠ?éÔØ{õìU?¸×6«*ù?À{BIýH?º³±@?{Œ?1°nO?¹Té6ê?ëªïW_Ò?º©_ð¯ø?àV@Ù²è?°xç/ª´?¶{*pkÛ?BþA¹Q?ÚH³°9?¬ÓG×6Î?Úª
ŸûL{?«cÓT¹ñ?•æEô^²ƒ?ƒ‡:òØÃ?áûȀ_d.?«‰;qÉ'4FGL J0934.3+3926?䙎ˤ@GÉ-ÀÊ`À:-ŽÚ"ö¥À<‰ì©&¥@}ÈoEF@i3]$žE?·3Øõz?Ž8èÿ³T?ÓþzÄÂ<@É"ž:"$?ïýqåöi~¿ä\u¡Â²í¿æɨnZQ¿â¹Ùె¿æöJ²È¿ïÿø¨ó©°AGNbll3FGL J0934.1+3933GB6 J0934+3926?ïÔiš aû?lf²®Ì`?RþÙ
qØ2?Fªã½ÞÅ#?q|m2Œñ?jRyÈï­?ïŠCF5Þ?‰>‹öÍÎ?Q›âÄÁ¶?cÿˆÉÍj?‹;Í\Yðb?†M¹(ïý?î¼£›hˆ?‰ NI?t·PvÇ(ˆ?dŽDñÉ©?¡žÜA'e?†E»úXfÅ?ïO"BŒÀ@?xzk¦¹4?† û]˜:?p²IÕ.uY?…}óÿÇWë?kZôdŽM4FGL J0934.5-1720?ٙ۱Ÿ¨Z@8ÃF4—·AÀ:åV"tnÀ<__á'@ 됚—?ÿ%"ü|?ÇÂЊ¢H?°³¢?–ª?îïŸËm@­Åñxô¿ÜÈ'ç%"¿êõŠèü®?ïþ@!Ù¶¿è³2ÇÓi¿Û,kãþ"¿Ñç6žË2AGNbllRXC J0934.4-1721?턮GÊÑ}?¬™ÂÔL-?]¬/aÅU×?XžÞa?³cÝ"^Ë?¬-'ò‰èž?î¿m>O³ã?¢ˆ›Å)ì?iüRµˆ?w—#!l74?¢wSû?–˜? í6=ÏV?íCf"Å"?™E¬¯u$ó?~'uI"©?lr×j·™Ü?µ"ÍvÇ«K?—êB%û?ëf˜»ã9^?§°%ß½Ñ?xd´Òø‰Ë?wØéÎVh?Á¢wiÛV5?§_Ȟ4FGL J0935.3-1736?æOvl@8¹'^éšcÀ:GäB4WöÀ<2Ÿèh3Æ@!mQ³¦á?û®Ð³Z§?ÄoH7QOÿ?º¢žA-?üG*{Ԍµ?ÿ·Æñ¬¿ïkÚ佄Z?ïõeݪj¢¿í†òÞ€é?Öª"XŸÔ¿Ô¾B%>}ê¿ç:R ß²AGNbll3FGL J0935.1-1736NVSS J093514-173658?홚Ü6qb?¯ÅËÁ{r?sJ³YÔèÜ?pxD¨fö?±þ}è¯&Y?®æZdÃ?ïeÔaâP'?'ò$	é߂?^Æܜl'†?o"4ïäz?'Yùï$¶?E]é&Š?ë©xˆ) =?¢k£×ü!œ?ŠA{õ d?€ZÌ''ì‰?¿l/8J?¡ÞÊîi?ìkÆ=(ä¡?¥
*£hB?›JiÊÆ?—¼ì|?µÏ3¶ðèP? ßp7à4FGL J0936.3-2111¿ä.¬QÐO@6už×ÆûÒÀ:¿YHp²À<iéæ¹@ é#mîE?÷ d#–?ǚ¶Äø˜?ÔÛ:£¿ã/@¢HåL"@E`í²v¿ïÿýF\I?ï÷{+ðHÓ?ìäS äQ#¿Ñؗü`Ž5¿×<ü_·u£¿æåÂ!øùAGNbll3FGL J0936.3-2114TXS 0933-209?îF½1ªö?§v½ê¸X?Œ;øÁƾ?‹ØÏüP?¤….µŽä?£klGâJG?ï3;•às?¡Ä³šò?oÀýd;`?ŠGÁ#:ùz?•µÄm—j0?›Ògþ͞?êÒ°q¨¯?©50G0%?¬ÕIXà%\?Ÿýڏâ	b?ºÿ×ÆOOà? óïÀi /?íBV|B0]?¢3ú"ˆA?yÁÎâÏ×?u/¦VÜV?´Q//ÁŒ²?¢¯ýö4FGL J0936.5+1847?äæ™/Dç@FR  ô×®À:®4|ßN°À< …S'wŒ@ÁÕh|Á?þ@¾kàùª?ʊÄê€;û?Ã*[]É´¿?øJÚ3½œ®?ù¥HÇD!Ã?ë£t'ˆÜ¿ê7N€–"U¿Õýu‹¿ÜžŠD<
¿ëP.Ë¿ª°#çF¡AGNbllGB6 J0936+1850?ì¥'}œ6"?¯"œ¿è§v?‰#ÔÓ*
´?ƒf0¥Ô?·²Ix¹
•?­Œ«z¬LÓ?íÉþ5³Ã?­šè{ÎV?'ئvã?"³Á¿??³+†p̽­?¨"œH'K?ìææƒyh?šâߗ#¥"?'LÇõ1÷R?…cOnf'‡?´;ÖΗ¶Û?•õLæ<?ê×à´=Üû?Ÿ'[ª]æg?¨6—? @å?''
òÿJ?½%®¾€÷¯?—Þrù24FGL J0937.1+5008¿ä†²?i½@GVºI<‰ôÀ:?'Á^ÁÀ< *#¿ø©@ GÏ!É@z䢬h?ÁS¬åÑ«"?ƒåä¥@+e>H:+@
žÄ½B?í´®"%â¿âÀ_×,v¿åš9҉¥0¿å݅TÖ¿ïññ\Ï¿ïÙ§'æøAGNfsrq3FGL J0937.7+5008GB6 J0937+5008?ïQ`1M|m?ºaÈít‡?}Ýƅ—§µ?y®Ï0ý‡÷?Œ¹iÕÂ?Š5¨‡*ö±?îü' S?ž¾<LM?p Ñ/}3?ˆY"?œg‡´ð¶F?—'óÞô?î{8~¥£3?Ð‰¬¦Uë?‡¿Zcí$Ï?|ùH"äõ?¢\¡|ªƒ?ˆ5ÌoÇJ?î©.8r§g?ˆ–&ƒªÐe?•áµlV}?€Up¶–?"ù(<>¼t?€+š`…ü4FGL J0937.9-1434¿î¥ÒPU"@;7Ffìž#À:v^$x…MÀ<o»^æ?e@ 
Õö›þ?ýæD·%?Äú`XÛ8u?Á¤÷Ãpƒ?þXˆøa¦
@
ä"¬¿î¶Ãvö?ï÷uýÞÄ¿á"&ÈÁ¥Q¿à8äl-P¿×oXz™¿êá´N_ßAGNbll3FGL J0937.9-1435NVSS J093754-143350?ïÙ`'×'?kõuèw?@è
À.RÔ?9õÚböÑl?q2½<uì´?jÀdoˆâ?ï¸~Oîë?~мŽFîã?>!‰®¯ž?N鷕ƒð°?ï¶ÏÇ?|ש]—?Ì?î¹1a:€u?‹-NÙ£F?j'G‡µíC?_¯"4?¢ÄÅsܙÞ?‰£
¨¡˜r?ïrô¡´œ–?uWwyœç?ZI‡UƒÝD?J	'CX?ù¦¨(^¦?t o¨V4FGL J0938.9-6403?␚®†T‡À!AMµ•x£À::Þ¨—c^À<;0µªq@?Ôó@@˜Ž¼ÆÅL?½ÊA¤åþ?­â~ðå ?ðXÑRm‹@éØÅ~yÙ?îˆ|:䝿äžr£hû¿áV™y¹*¿çôÀfŒý¿Öý'aĖ¿æµ¾§6AGNbcu3FGL J0937.8-64071RXS J093850.5-640334?èÃ՝sŸw?¹•‡Œ?ŽÒ?~iÁ'Á8?tO_­O?Ëý[€óyƒ?¹1~w¹ùO?è<¨IámÓ?ÃÓݍq?Qœn
°»?`á^Uî=3?Îê?Ÿž-Q?ÃðÏ~¦o?ëÈÿ(œ¹??¡<όÔ5?…9ÜÈŸG?pwYööK?¿Ë"¢? G:ór÷?îZ¯¨ã$h?†y@èÇ	?rˆÙçd??a4‡³W½?¨êAÐÌï?†KúУ0H4FGL J0939.3-1732?ï¶=ñŸŒo@9yØ¥H#…À:
tÓ³¬À<Yõ2F¤@œ' PíÙ@'%IÆ?¼µ¿êç!?½Å°"òô)?ÿη«c@ÙÛ]3a×?ïýCWm¥¿å©?Êjå¿áÒ¯')c¿äKùӖª¿æuQ@9¿ïèÎ?ézAGNbcu3FGL J0939.2-1732TXS 0936-173?ïçº&-)?cŒ lLÞÒ?2œìÄÊÖ^?/«…"B?eò<:a|ø?bš
Šðǒ?ï»fÿys?EÂΉ¬¡?@®T³=¡?Q'>i>Ï~?€&5<s/x?€5t­Ž~?ï8ƒ"¬s?€øI#ߪ?pQ¾'ò?b	oïs½Ô?˜U,	ÍF?~(p‰ú†¦?ï¨R®Pp?iÛs•BÂ?bãðâŸF?K¯nõ²?f3<4?g~ÚÀâ4FGL J0940.0-2828¿àԜÏÙò@1éi ­ŠÀ9ùÓ°ìœvÀ<3ÅìÞ»@z[±×~@£ŽDÑÁ(?¸f¸³?ƙ˃ ±P@Mí®Ä¤	@Euà¬Óˆ?è]ÿÅGN¿ä` CAs¿å"—Ú|¸¸¿äy;.ª7¿ïþ—J4¹?Â<:˜Ø(¡AGNbcu3FGL J0939.9-2831TXS 0937-282?ï—p
ªc?†s…Âm?yCAþ©7?y',õ–"»?{·u˜?{%­ËÉ·?!—³ñ?p]¾\À?R‡»y	t]?bã´±6?‡*ñÕ$?ŽƒÖ½‰â>?îz§j•Ö?•"V<!ó?'®Ù²}y?ˆ^ì÷aô?¤°è°å?Ž¨–.O3?¬}Ï?p²ÀDÚä?f&hw™¾?Sü+6™çx?†ÕzÂ¥ø"?m9³:pœ¡4FGL J0940.4+6148?æ|(Í~£t@Eš:э%îÀ:ž:'ÌE¾À<œl%Ã(@ ÿƒ'ǁ?ûþ FÇd®?¿[äØ1Yê?²ùÞÓµtA?ôʇx.æ@jk5Øÿá¿Ü¡]Þ,›"¿íNj¼[f¿·Ãñ®¿ÛiÝk폿æx`ˆ"?Ç7¿)ÌAGNbll2FGL J0941.4+6148RX J0940.3+6148?ïÃÕÛÒE?w‡Ï¡ùX?F$»J™?>óvq'@?{Pôú­Š`?v=@ãõû?ïhl|æ<˜?¯–u'ìO?P7ªžÒÏ?\ƒpÄíÂõ?'îþ˜Žù?Œ /ïùRÅ?î…L©…ž?'ë€?l‡?dQ‰ï<ŒÃ?Y¦¹`ÎPM?¦f%ÆsÝ1?' XÄ?î¸übëv?‰îÏ*pún?p•—'õ¾l?bPÝ÷2"?¢]†ß ¹?‰'w<ù»»4FGL J0940.7-6105?ä¸0
À!)Es§˜À9èy§‹Ê¤À;ڽۘA«@—Š«j&@æc[ïêß?ÁEj˜?Áâò=ŸÀ@;†Eÿ¾'@	C\($¿ÝÇkäՂ(¿ÓENJm¬¬¿æ}å=ÜÚa¿ç¯žˆì£,¿ïicÁpx8¿ïÿú@ùDzAGNbcu3FGL J0940.7-6102MRC 0939-608?ï-øe½r?'õè¥Üd?v÷²aéÚ?xYÍäLr}?"ƒÅ!Wp?Ë¤>b?èZSȕ?ĈÏ1aç£?k\Ÿ`V_?{°ËÖKµt?Î(ok.2J?ÄtúüŒ?ìnž'?ž›L¹»7û?—}[·¬?†€'RúGƒ?¶É€aÌ…?š|?Á²4?쎋wvÊ?•5µ'Ùž_?—®Rð"é?€<•7Aô?µ ¨;Æx?"‹Åù
hÏ4FGL J0940.9-1335¿ïþL?QW@<lӝ¡fÀ9œÈ\ûƒ™À<'Kžd¶@üËÙ1ß÷@g'ûÈbÛ?²z|öê?½iIśÖ
@‰—Þ®v @¥o;¢?иœ>9¡Œ¿áŸ=ب£¿äNô‰u_¿èWÿ›V2¿çþîк˜¿ïùö€û=#AGNfsrq3FGL J0940.9-1337TXS 0938-133?ïÈR–bÌÁ?†>o7dÙa?EÙk'Ib~?COù	K½>?y‡\Ps?…¯)•H6?ï·ò"·Ì?%ùb+›??!<˜7Õ?O˜ß}z-?%ð-Ke?}'¥rt?î¬}=©©?—É7ÖA%?t©—½…?l©¥ú@ºù?¢¢ùM'M¾?—Æð!'­?ïÐ$ò4<?`smUíßÌ?Iã¼If¢?8Ãþyç²=?t»jnXÓs?^hµˆPi4FGL J0941.7+4125¿â×XHÚÁ@Hp}€^_1À;@·E|À<º¢ô§@£Nçï'õ@q<ƒ>?מý0ÂÁ?å
ƒç€­:@È[TŠœ@
eBŠ¿¿ïë"ÌÐþ‹?ïÿì´É È¿æ/ñ)£gy¿êOž£Ä•Ç¿çõ2F¤¿ïü¾â©WþAGNbcuGB6 J0941+4121?îæ™Åù?ªÏR'²? ¶I[ê]'?©e1vêŒ=?\H}M…?mâg'è%Ÿ?æVl€ä\?Ë$%ÔB?Å(?L£7?Å}7iG?Á~°]ì|?¼¦n鿏?êô2õd¥c?¥Í×	›w"?±!"ãDR¤?ž‹'£NÙ÷?·=Eq–'E?š eÂa´?ãýž¦³=?¹6XÍÎ,¨?Òhzasw?ºO6áÊê?¶uú­D˜=?¬˜ü¹Ôm4FGL J0941.9+2724?ï¯CãÀÀ`@HëC,¥À:<éhSÀ<Œ_Æ94Õ@ûˆ÷5=@-'$ZR\?¹ùÛßËhZ?¸r*rD?ø§{‰äð@	É0àóu?í ¶ž¸¿à‡)T ¿å:óṘè¿é£L Â'Ç¿àn—Oß¿é$Læb AGNbll3FGL J0941.6+2727GB6 J0941+2721?︪[.?‰l:\<í?Jç ¤|n?JY
úu?€_Æï.,Ñ?ˆãɃٻ?ïwd<_>•?‹j÷ß/"?S<îŠg?`óý­Áîƒ?¿X":‰u?‰ÇÝ(´C?ïRä<|
?ƒ=‰ÝæÞÝ?n+jr&¤?`v³€q?™ÐA+"9s?€ùý×&äÉ?ïpÛOì8?uû;9ì/?~ן½a?mïg"?"»Ànæjê?mêâžéJ4FGL J0942.3+2842¿ÇŒöE¦@H<'RT`ªÀ;D€'q^èÀ<È<){úL@ ¿›7©d"?þ,7«gø?ÆViGt‰?‡ºhµåÄ?Å_<¦y{í@Pò‰ø¿ãù`ÃdC¿àÆv;Ƭ¿ãÈßëb¿×:,âMf¿á°@¿ã°>¿ÔýAßAGNbllNVSS J094223+284413?ï"CÎ-0?ƒÞL`Qü?@-n'm?>^£Íó?‰÷+"Ah?ƒ&ÐјöÊ?™»×?Š¬˜Nfd??ñ%¬o;?Ny7EÃ?Œž"ÜÛÚ?‰æK=Rtn?îc¹»À"•?‰ö¥ÒÄ'u?kna>>?Tè°ª]Ã?¨
~0¦?ˆ¤æSIÖ?ï2<Úè?‡g)²¡?\¥!½‰Ÿ?MobPž›?œofHÒ5!?³ïñÌ@F4FGL J0942.3-0800?±í™ÁŸ­@@'1]pŸÀ9—2éaX
À<^6=@e¬|`C@ç¡di6?³m0/Î?Âu'ÿ ±ü@AÁÇ@£$fˆ ¿ÁgncµÜñ¿Õû"¿e=¿áƒ^nË:¿ã@*'zÁg¿åb¼ù2±¿ïúÀZ΂¯AGNbll3FGL J0942.1-0756PMN J0942-0800?ïÖ¡@©†"?f4©‡Ç?Ö?Z²±l"R?S^Î\ƒœv?lf xÜ"?`¡ø8(Ò?ï²—ºR³?ƒhÄòøa¤?B"C×CÈu?W+mWƒ?'NåÓ÷?'+2±ó~¢?î¸ÔöœR?ý¶Gø…#?‹ÍOj×|U?†ÎÀ"æ3A?šþ¹‡€·?"‡CkÝÛd?ï½·å°©.?e/LEM
?L"þHÙö?7îbD"Î?}'mdND?d#ÐÚc4FGL J0942.7-2028¿îUö^Áj@8	WG²JÀ:Ö½A>Ž±À<'›Ø'@¥:=h–A?þ£ð4°áµ?Æx»þsc?¾iAžA/[?ø²'¸#È@ÿŠÏ§G­?ïîá"Úíø¿ÒwØ¿cm¿Ó:4g¾€¿áÄÏ9°%¿ÝÀ¯óx2A¿åÍôIéXAGNbcu1RXS J094237.9-202720?ï*£Y»}e?›êlVc#?WJ¥Z|?N€'9?™6ó6õýæ?Œ¼àæÎÜ?ï‡ÓÍu?•N.ÌRt†?]72ʲ?dá!bÍ÷?iVòY¦f?"uÁCLl`?î?/ëÒ?'Á3"Vm?w-OÇâP?dÞìL¯ëI?¬¦d$!&‹?Ya{À‰?íp	Éҙ‡?°h"8d«?€G
åþå?k´hGEÂ9?²vÏô«p%?ŽºoQ84FGL J0943.7+6137?æ -r‡‰@EÑ(9-ŒÀ9ý,ðùÒ¿À<q
À²ã@íúCR@Žm=ðüW?´ÇV2ç‰?Œ.·´è?Õ¿~°Š!@Oš¿ßS?ë]F,4;q¿Ýq¹`‰W­¿éOt.©6¿å¹ôMDVq¿ïÿøãú?íÑØÀ  AGNbcuFIRST J094420.3+613550?ïíjPÛÔf?~v5Œ>Yy?Ug5[*?z.Øë?OˆRyø?U‡p™ƒ(=?ïy5ÿáhš?œƒò±]Ì!?JÖQN	‡3?aì€ü'Ñ^?yb ¡?›ðÔ
7ñ?îÕjµL	$?Š0Q›ÍE¦?~^éävpK?uã"Ü"†¸?ºîÝa?T?…Wo6F|¬?ïëµx?˜?T.ÑæjDÆ?S'¾"íè¥?L
æÅ2ñ?U{'åñ?Dªâ?J4FGL J0944.2+5557¿Ë…»¸Ÿ»"@FûŽ\NµpÀ;q¬O~ÃTÀ<üóæIî@—wȹm?ý–¡G
Ë?ډµ@>3—?äûë~Õp@—ÕÄÃ?ñðtY™#}¿ïýv:ÂÊ?ïÿÄ}îB¿Þ¿EE•6¿ámžÔký¿ï°B¿êfì"¨vAGNbllNVSS J094441+555752?í'
é?¯Ï;xð6É? W¥Œ¡Ú?žIUѶg?¦‡˜ÓÅh?¨‹÷£Ir?ÜƇ¿˜¨ù?ËUÂî«i?Ø!©¹Ç?Ìáy:)V¬?ÆT®Q{:}?¼áNïw¡?織ãG>í?ª¹I²¼?º@R›×Ï?žäL¼÷c·?Ãùƒce?¤K¼¡2ÿk?à§àˆ¼Mp?ºK@£ÑYÚ?ÔèΆmc¥?¿B˜:Á{+?ÎàÐ4ö?©°;'>c4FGL J0945.2+5200?ä1|½sq@G´"ÀÀ:YôNñ՛À<•Ìe÷@»MôU@Üʵ›?ÀÊóÙ¬T?ÁÛÕ~L69?ú˜¸É	Ê@[q¥ß£¿Ôlbñ¼Æ¿äˆ ËQ¢Š¿éx° œB@¿í•Œßvó|¿ïú¡†Íäû?ïðÝî]@MAGNfsrq3FGL J0946.2+5209WISE J094452.09+520233.4?ïß>ädãö?}ïꯉ?YÚ©4éÉ?pŠóšYZ?cÓǧz*?tF{qhŒ0?ï]y†]&?¢Œ›^ߦ?Tã@¦T«ñ?o/ë…&{?"›3¯'? ûn<‡¦Æ?îù$jê"?"¨"gÔN?qÁ´?‰¾Ð?`R»ªq€È?œk'ÍÀ?ƒ%k°´ä?ïÜ[s Ë?_H?¾ƒ¨?X‡ ×{ì?Jkš˜ŸÅ?g`âCów&?Y	—è‹'¯4FGL J0945.5+4635¿è=®ün•@Hf¼b~À;åác\ƪÀ=—^Uö­@!ÏÎ_IÀ?þº©êIµV?ÅŘ•2¿¸9ë‰%ƒ?í–?aê«°@!¼:®Q¸?×A¦=–ä^¿êWvßZn¿Ö·¯™¶¿å®ùèŽÊ3¿ÒS^a_@'?ÍãEµ÷AGNfsrqB3 0942+468?ëèÀ?Ǧ7p??pV›åuBå?Ì;'¢?Áã´²æ?Ç#½ÏáB?î|²Á'j?©¯6~sØ??osüR*ƒ?€ªm"ñh?¦=®T!¶°?§ø¿M`<?íqøE˜?•U˜Iw£'?wãðü?l]hjU÷?²øÙ7Ìÿ?"}rƒayS?íVÄÔÑ<?¦¥tåX¬Ÿ?g#Qñ'°ù?cRC[ÿqþ?´ÄqÍ`—?¦×äûlÚ4FGL J0945.7+5759?áYÆDóO@F±3 @|ÈÀ:Âð\À<'*¢jùs@[êæhTR?ýþŽæ¸0^?Ãëv?Úá?Í5³Ö†´å@üŸS @
…ÊúåŽæ¿¹)LÕpµJ¿¼µ,òý8%¿ØR'_js¼¿Ù;}8ºÝ¿épà"&þ¿ßVóé	AGNbll3FGL J0945.9+5756GB6 J0945+5757?ï=
8\­?'KH"y?‡uÉ´"UŸ?ƒН1­ô?‰Fè4l?™?ˆiŒðÆ0?ï‰*uA?‹<Šm®—?Pf9ۜÅ?`lˆ±Ìñ?‹³°[t(2?‰‰&-Ö~W?î9}®L+?"›¿"&M?'ö>61I?‡ŽF'ÊQ'?¤.}$µ?‹b^# ?ï>}©þ½¶?yҝßQT²?pÿ|:à#6?\IŽOΝ€?"ðk±p@ƒ?v§ÙñÅ¢´4FGL J0946.0+4735?âÚEvµF§@HW<ÈóÀ;ŒDÄU/À<ÝêPkR^@ ¯7eœè@ËHZ⤥?ÁY°àÝûÉ¿¸ö·Au@I?ùìÅÛA?óc-+²5r¿î~¸—·¿bø;v´Îe¿ê½¦îí¿ë_:øúRA?Þ]JÿÓ?¿Þ3xgðª"AGNbllRX J0946.0+4735?îQ·yÁ?µYîá¦?….÷é¸.?'‡? —AC?¥¢¦õã6?´Ù³óŽ/°?î&Qxb`?°4ÿd3žf?'Sñ"›Ëƒ?˜a‰¿z(?ª¸žŸÒç8?¨þ1ŠÜ_?ì‡-? Žó<¢ù?•ón'ÌÙÊ?ŽZiÄ
C?¶Jóë`Û?™m¾¸ú4?íVžHú?§J'æž_w?z·¦Z¢?C'X4?³Ÿ"Ÿ-?¦šÒ\p´P4FGL J0946.2+0104¿îúz[!@CH
|ZÄrÀ:¶ßh°ÄÀ<[@dtß@!T)΅‰—?ü‹'™Ù?Ëùwœn¶?¾Ö?;‡?ô›ƒEW"@¤}M]«Ø¿éo»^g"¿ÝÕÿ™'Ú¿ämð‰Ó©¿Û'/'y—q¿¤ûg{¯¿é˜=‹ü£AGNbll3FGL J0946.2+01031RXS J094620.5+010459?îU› þÂ4?ž¨ 0yL?b÷Qx?WTO•ú½?©vØؓË6?€lÕÕV?îÏ­ƒà©w?£½ïÑDé?hg-A¯£?xTÔV»(?¡~¶_!M˜?¡yîóÕ;x?í*ÏƝ?˜´ÔÚ¬èU?y«cLR?f=–¢?;…?µ«–R!?—‡±V>-?êW†ÎûLK?¦º=‹a5Þ?s³[öI¹?nf윃?ÆIä`?¦êDëQ4FGL J0946.6+1016?×=8pÅ÷@E·<³åu:À8†'M!À;ק{¬]@æP4JàN@ÀÐ$p!Ñ?Ÿ|/Ùêö?´Û³@^çßwÊ<@´Çç4×ù?ïо"$哿àð´"†è'¿æ—ºÁÝZ¿çlÏ¡"c¿çµ:uFÔ¿ëëJ ŠAGNfsrq3FGL J0946.5+1017TXS 0943+105?ﺮ"‡M?€&øäN?P´Œ†˜"4?Mp´"k@?~{˚Ò8M?~Ÿ¥¡™É}?ïdâ`×Ú?x6"øR?UGIþ/?fÖT<ôì?'
ßp~""?¥	"0?îäf¿{2r?Œè:|É?zëIñ???roJžÂQv?œìm>aû?ˆ­Àb^°?ïߜŸÇ?Xç¶wÒµ¢?Vå~8²˜?HºÀ[QÇ?dð£Þ.©?RMvYîšY4FGL J0947.1-2541?Ó|ïl{@5Ý~Ë·úÀ9cf´iÿxÀ;Üå`A‰7@Œ•]õ©?üɕà§?°Xù:>?¶w%ü=ÿ@
'¿}Xñ3@
9¨…oÁ?ïò'x=?Пà·õ¥¿Ô¡â=wYÔ¿ÞgÚúâß´¿ÜÕÓ;{׿à 4éì˜AGNbll3FGL J0947.1-25421RXS J094709.2-254056?ïÑ["VnM?r	ÈHÛ®q?Q¡›Å?TL€fÌlz?réïáçý?mØƅ¬e?ïnüSmÐÛ?l²RØkÃ?avß­ämÀ?qÀ‡}×7Ý?ã39­Ñ?ŒxqOO"Û?îëÐH²*Å?…9è2×5®?w0Ó®=´_?nš‰J§Ú¦?œ¹Áþ+:?'E˜Ès¸?혀*ûÏ?•‰ó÷È»â?ƒþŒLdJ?nÝÈùñ?°ÙžÖž4ú?•"׌©5%4FGL J0947.6+2215¿Ðüœü®@HJƒ±ÐÈÀ:ðë€ìújÀ<´¹‰$@µE@ûZ~ї?˾_·¼^?Ðe)O"¢'?ÿý&g@Úp'ÉôU?á΄'Ai?Ðgâ<u§!¿à"Ä"ïï¿ã´zÆo»¿åˆ©©µ¿î•³€ y]AGNbllTXS 0944+225?íñŸeû¯|?ª,Qo^x?ƒTÏŒ?yÓ§ã]?¬ZAå?©"‰=U?ï6B±"õM?'îs¬ä¶?`·bh ?gƒ22-<Ù?— ¹¯_‰Q?'"¹6ÊûÛ?íÍîÚÍj?"0?k–Æ?'ØU?4ÂKÔN£?«Ë-!þ?^³öH—T?îe–´Ñ?†ÙÝÀ=Ÿ?ŒÜÍõ
îa?s£ÁSʇ?¢p³s§\?"Y-poÞ34FGL J0947.9+1121¿æ­J•@F¸ºÇÀ;n'D:ÂÀ<›@'§@ »;'HnY@¢õ}Åþ|?¢#€ã•;¿¾Ìô9ù ?õò-å˜î@Ó£¬íßA¿ël™ñ®-¥¿æo"‡¹E¿éÍÝ~냿ÕòŒ–›¸¿ÕmË"°¿â=v:ÂÊAGNbllNVSS J094746+112020?ï:"óˆ?}"ôyõ?g©…Žì?j¥y%´´¯?•¸[0ÝŠ?eº_]9?ï'ܲ]?
ÿ‰kº>?ZÍÍêTÌ?oÎP¡}ñ°?™WŒá	Œ?›lËù?î<e~æ–ø?'"ñëÐ?n¨ó´WÉ?]júG½J?ªOÖQà?x+Cyҋ?í«'H¨?Ÿ"׌NÒ"?dâé¥ò»?b&¯è‰
ü?²¸¨‹*?ŸJoíÒj4FGL J0948.6-0338¿Ñ;ƒêëø@B!ؾr–öÀ:ò6†¤ÊOÀ<|›U[|(@¤L9µ@R§åŒ·3?ÃéùÃÐϼ¿¨ªWVþêV?áõbLM@~á8>µÈ¿à0(QWáh¿Ùgð>Áܯ¿éÕ2ÌÛæ¿Ûà?:¨rz¿ïÿÙ3ã\[?ï¿xPs¶AGNbcuPMN J0948-0338?ïªÌP ?©ÑŸG7¸?sQqN
r?©Ìcz³ß?wŸƒ	¢Z?v5µÉ½ò?ïgX^iØý?•çm'Ö/Ä?Q+ær×.?dP^aä´\?'ûñt]³	?"t3om?îAMË"	&?ü~J1Û?5ôÀæ—]?tèñß4?§¦¥ÇÚ?¯Òn>M˜?ï‹ûº{?tëºó4£?`¶Ï` ?RüïîÝ?‰Ók¹Z`?s
6PTV.4FGL J0948.9+0022¿áìCrpŠØ@C[¹pޏÀ7Û:,K¸eÀ;ÅÀ–]¤÷@~jM¦¦ó@Ÿ¬EmÈZ?œX¥f4?Å&J*øQ@$»`Iì³@O­·4¿ÑA¹my*¿äz™ú©¿éšñB¢çÌ¿êÐ3¿J-K¿îÇ·ºã¿ïÿ&¼,k™AGNNLSY13FGL J0948.8+0021PMN J0948+0022?îÕ½Ü:Í?¤NCû´pX?¤9ûÚzǶ?£^VâÑw@?}EB>[ñ?{‡…õäq?ë:¦Öð¼?ō#"-EË?²›-™n?À¶g²¤œ?´$.CL†h?²ºbĽß?ìh©¶J‹?©—M¢ºb?­}¬*`5†? ÏñÐDýà?«÷¸l«!Æ?¢ÎÌ)ئ?î0ê2XÄ?œ!ÂzcÎ?¤1')Ô.è?™V­b`aÿ?'€ka?! ?7`4FGL J0949.0+4038?Ø-ÆTì)@I'½{ 1ÏÀ:{ôšq/îÀ<âž43@I²dkº@ñ^aµ&¾?º7U½¿"øæ'´?ÐðjÌ&´ @¡ïDÆÙn?ÎòŠ÷jZ<¿ãZK:õ†¿ë&qN õC¿ãâg3B¿ã{.¶Ì°¿áäúÀûÞAGNfsrq3FGL J0948.6+40414C +40.24?ïÓÛלÝ1?uÐ+cÕ?U'çɓæ?PZ
€X7r?pÈR·Ÿ~?sm8²]?ï¨BDy¹?"Ñ…W!¼î?=å;Àd;ö?RüÁ<?…6PÞp/?ƒ¶RÍ%x~?ïò› ?ƒç覧ŠI?kÛCDu·Î?ag‰¯†–È?˜ÁYCýI?'O¦úÃu?ïܸÅ|hí?VAzø½?Rkì*¶??w¥²µ5h?jD€Žþ?S<©—ä[_4FGL J0949.2+1749¿Ø/&úüÇ"@G'«!ZÀ:Â㨱d'À<ˆ–&G'f@<ÁQnˆ@öå¥
ç?Å.Bž
A¢?Œ$P
Öϧ?ÂèyfkK@ø÷2Q
¿ì]ÒC.S¿¸¯ƒ»¶Ð¿è¸5›Ã?…¿àó›}Ê[-¿ìE¶ù%ñ+¿ïÿÉ–oAGNfsrq1FGL J0949.8+1757TXS 0946+181?ïÍÚ¶"Ÿ?uUr½~Dé?PPÄ׈|Ò?I!ñ^L"?tþÍnۑ¨?s¬Çíˆ?ï¥ù'"·?‰ÎK>†ò«?:rB[¯^=?PÔÍ¿·#Ý?…®,ȁWO?‰ªn .À?î¬}	ÿã*?Œ§×bk™?~@R,cDu?t§nÜ!?¡p%ud¯?ˆ',›¼$µ?ïתE"ó[?\¥ğšÜ?MR:ó	?9|S¥]?p€–.gâO?ZI<'Ö44FGL J0949.7+5819¿Æùy—àJÈ@FÝ]Ý*èâÀ:=çi0EBÀ<x5k×Í@Q¡?*bT@Î=EìÏ?º"tôô‰)?¶ûOþ+OË?ørÀF¬Œ»@zùdZr'?ÜÀÄÖ´,¿ãG(é-U¤¿çkÄߘl¿ë[î¾96-¿Þ¿â®‹n¿ïû›ûs©AGNbcu87GB 094609.3+583301?ï¿A#¾?¨J"hÝô?^neç–wã?'ÉmP\?xàEü'ù?¡úÌ·ûÑë?ë7¹|?‡e3ŒÀ?H'Ù16'â?ZèìÐ͸–?‹Gžþ7Æ?…2Ù?ï*@â‡&K?€åè¨z¾?lhª8/5?Zý:˜6?—*ÎnÔ0³?~¶/aûs?ï­ïš×‡?iuÅõA›Ø?frŠã1fà?WP+˜•?}Îí"£Ëù?fŠµöÚ4FGL J0950.2+0615¿à£Fñœ@EFA,ðúÀ:Zˆàä±ÆÀ<n;è
šó@ÐÉéC?ÿ`_¼(:?Á ¥¼è~.?ÀØÉÛ*Þ{@9}I׺g@«ÕÄF™¿ïÈ͙{f©?ïÿ3¶>ì¿â¢çUåã¿Þs²LîÆ¿áG§~´ì¿ïûÇVkF AGNbllGB6 J0950+0615?ïÞÁgŠ#	?c°ñò,Îö?R7ARIâp?R`x™fYÇ?h"÷̸s?\ŽÁeCe»?ïk‰ïºC¤?™Qs½ëÞ?\$¶ÑRÎ=?i§´,¥Öæ?Ìv›¢^¬?øU'Ô ?î—Áæþ·»?ˆ°¶Ü9½ö?vOuµ&êZ?h')ÖwÄ?£¹òÙo¦ø?…ÚýUWj+?î9{d˜ü?‡õfqt'?ÞÄõ
?w"Óòe–¦?¤\ÚSõ©?'»Èq®ó<4FGL J0950.2+4553¿ïÒ*òiP@Hß`|A™þÀ:¸7êRÀ<…Q(ÀB@ŸTÄ}s?ÿz"¯tÍ1?¶-z¢§>?¯6¨¢e?ؓÓ›fù@<ȋ­?ê;KÀ¿n¿ÑÄÝÀ$5¿å4Ô#&¿Ò¶´DÁ¿â2«ž~Û¨¿áÊFà!AGNbll3FGL J0950.1+4554RX J0950.2+4553?ï‹â¥Fm?€G%ºùc?aß4Ut"?VlvX'¤?ˆšI™Å?}µ	à¨ýj?ïm‡àÔ^§?Ž_Êùj?X•Ké^?g`¶¯ ?Îzµš?‹êJêä?íëͳ(î?'AÄ9ÐÿM??Äê)'J?ró"ýʐ ?¬ó3'õgT?ŽM"©"ãÜ?î‡óöA&Q?‡5þ[Á^?Ž9Ã<¼?uôsF	"n?ŸäŸ²=&~?•†jÿ4FGL J0952.1+3932?ì–Çùd–"@I€Ž6FÀ;rð\À<Ø£oqY@!‰Œ{ÎØk?÷êÐ"¢§?Óå¿âÙ~Œ?ÌyÞýPù?ü5K÷OWV?ô ˆ­Ž¿ïÿÿ" 5•?ï÷‹Pb?í€ðÀÇÛ̿ӊi%¡_¿ÔÌåÄ—¿Ýx(Z½ëAGNbll1FGL J0952.2+3926RX J0952.2+3936?îðÆ_Q—ò?¤Ààœq0A?b'ò¿–ø?cvúää_¥?Ÿ"õ½Ú?¦?¤Šs¿YÇÙ?îƾô]Ó?¡Î–úë˜ö?pw_øçt?yØBÕB?¡¸-›Ø? 4–I2(?í,YEqfÂ?˜úÀ4(ƨ?‰oò½>ˆ@?' `à?³o7|Ìøê?—Œ'±eÀJ?íÀú⌎?¢;øÏÇ¥?ŠW³?ˆ3æ'Iní?´	Ô¾
? öӍJ4FGL J0952.2+7503¿àãÒhJʲ@BŽÌ¼Õ,À;}§´æÀ<÷;«§¹@#2Xëÿm?ò:¦ú«,i?ÜHñáYKÌ?Ô¶VÿIh@¤m'Lž@7mŒöH?ïOÄÞì´õ¿á¶2 ä|¿ï¡±`_¼(?î»4ßZÃñ¿ª]{íñ¿Ì‡Ú¿Ô–ÆAGNbllRBS 0804?îú"ß½1?–0ú€Ñߣ?l°÷G'í•?jFÅê¯?%…y<?"éèù‰?ïLeAo™å?›dÂèÜn?Z'!'sÀ(?vL;àØ
$?"Ê5¸õ‡S?˜¸æx´(ß?í
Œ\ùµÕ?œ5L©Ù?ƒ>}¥‰¢?sI;¿Ll?µ+Íx ?šÔ&‹èa?î"uq+Äo?¢·=Xö}B?dãUƒ£3?|ÙÏWë×'?¬Šs•	…ì?¢o瀏4FGL J0952.6-5048?ïõTEÛ	.@9¡vݬïÀ:ªî!±*°À<2kÛñ,þ@ rUãâ=!?ÿD*Lä'?ÎۂGB‰½?ËÁЈgB?ýIƒ×u.@	qÁpÎ\¿ï'Óa'jv?ïøx·¡Â]¿ÔìKî¿ØCe'Š,¿éý7%?¿È¡ð•©ÊêAGNbcuPMN J0952-5049?î[Ôÿ"ó·?£7Ò­'
‡?k*»Õ£K?g«'álJ"?¨IfØ?¢¶z/F§G?ë÷ݝRÔ?ÀUrÐWÏ?d®÷bº'Š?}xÀǺ¬?ád«ÿÌ?À!(³æә?ë!ƒi$;'?¤`^®r?ÞKÕǪƒ?[œÂû˜?Á^(à¶e?¢)O'?î6ò]aԌ?Œo@•Çã(?xf³W;W»?ei…çŬ?©"¾ûLQ?‹òY׫8E4FGL J0952.8+0712¿íÖÒ(p%q@E£?á—_-À:ñùÌàÀ<¢Jmâ[ª@ IúõÕ?þHåL"C?Ê¿Yòª?Ïã}h`'@]ˆ~¿"À@Ën–™	¿ìø0Èõ§·?ïõ>¦-ü"¿Ø"GNNí¿ÔžÒn¥Ð¿ïþa?ïæf¿QºAGNbll3FGL J0952.8+0711SDSS J095249.57+071329.9?ï6O¥¥×+?£^«¾X²æ?‰¦ÝÕâ?‹Š²œæ
?ˆÅ8À¨y?¢i<?W¤?ínçÿl;{?°–ˆ;Ê?'it½Xg'?Ÿ²!º
'@?¯ÜŪÂ?¥1Üè‡Õg?ë´L*ºf§?¡§Úê<ø7?¥5 ƒ8ä?'ZúԀ
f?·ÂÎh‰Ò?™Ÿò
pøÆ?ìÑ#M÷Â? WÑUà	?¥ðèÅ­.?'¶
hzr*?´Á×­ka?™J7枤¼4FGL J0953.0-0840?ڡتß@@óO?Ù3ãÀ8d.˜™¿YÀ;n­£;ÙË@ßn"³*å?üכ'˜™?£Ú!þNò?§Ë
te@ždoa'@
v4‹¢àë¿ÊæW¸M¹Ç¿Ü{±|9av¿Úä1ò¿Üžt?¿Û#'K¯¿ãO"þ)f+AGNbll3FGL J0953.0-0839PMN J0953-0840?ï­ÔIŽU?|*'ª"_?=eöWà3 ?3þ7Ï`?ƒŸ¾
hå?{§ÀBÇU?ï'qC´C?‡Ýç½~ J?K|A"ìâè?Y/ëæãæb?«Ø•Ô!R?†¯Ãë,À?îÛ_l¬"É?'쮼ç(Õ?vl?ory°?sÅPÞøk?žùŽèK?—Ó­'?îÙÀ!E	a?«üͶ7?bÁ=ÔÍç?Pl¦Cë@»?¡7êmí
?Žäz…¼Ib4FGL J0953.4-7659¿Ô©+|xUÀ1Š©Å`ÇÁÀ:½c€ßÀ<`wç˜*.@ ø£8bG?þ¯(¬ÇsÇ?ÎÙh¼ûî?¡·×GO÷?Ñí_‹Íÿ?üY˜Ý±÷^?îz	{©ÄŠ¿æ³"µ!¿ãÞÞyÈn¿É@٘b7¿ãûD^Ô¡­¿ÇZ<!~|AGNbcu3FGL J0953.1-7657cRX J0953.1-7657?ËSÒd?•-æ±õ'?K=¸mÈJ?B0ͅ[è?¥VSá"¯?•ûX©E?îµ' ˆ:Þ?¤0?e7;‹›º?oì+º lv?£ZG˜Y?£vëüZ ?íob€­?–{‡íù?u4[Ô`ý€?dD8'l?³3¿.´‡S?•iØê‡N?é >÷0I?£ KّY?‡_V™Ùpª?w<
ã°9?È	F…§Ñ?£TÈøE2³4FGL J0954.2+4913¿Û7€ÓW´@Hɛ^•·À:¸®.|NÀ<iU1Š¼‡@!¼'?ò"EW"%Å?Ë*D¢s?ÔÍ¿Ü#å@
)
]Qï?þ%2êc
¼¿ïêzAå}ž?ïý³^f¾¿ÙÊɝ}u?ÒóbÎ+qž¿ÛV¿\W¿ÐtéæAGNbll3FGL J0954.2+49131ES 0950+495?ìø'Ûâ^?±ªóÂÊÂ?™_[eVÊ?"þîBò"?±ã'G—\Ø?­9¨"
uG?î'&è"+^?¤;ð"ÍZ?€mŠi΀?Ž.{à9ç?¢Â.ãiÆI? ý"­r³?èÿáƋé¦?¬Í¹†¶ñ
?³=ƒþ¢UN? ÒÙ5Œb?Âa¶æ.¾?¥œê·Ñ¡è?é2Š¿x0"?²¿b0Šwâ?˜GŒ~Ì-Ú?'A€¡,ªù?È,ãrE¹¿?²äFM@&4FGL J0954.2-2520¿ääMÕJõ@6_Až0PÀ:¢Iøq–EÀ<~ÑF¯ú@ /
Å"?ÿ‡šÉD'?ÄqÁ¹H`—?˜Žd.d?ØÁ—¯@÷
ú¯ß?ïÿ!ڛB¿Ür½'ÈF¿çp4摙ñ¿ÄP'à™³E¿áHÍcˁs¿ä'gÁZRÝAGNbcu2MASS J09541965-2519588?ï"Ú¯—@?"ÓÉqàJ?Y}kŠ~Â?P¹^¹¶¹™?š26_Gù?"fëÍ
?ïMÉ
Ù6?'~ÞGQ2?Q™ï®z¢J?Zá¿J3¨Â?•Bçã]/:?'Qõd?í Uô?"sò¹?|Vø¶T0j?i¥ß¨ƒ÷=?±7ç㫳?'ó÷¨³Dï?íœKXcp?ŽÞ¶Ç{u¹?"nÕß,{$?oŸ#Öçu?°ÌYWU?ŽDz{ýü~4FGL J0955.1+3551?ïüãŽbâV@Iß°_®¼AÀ; ˆÂ±ÀØÀ<ôæ¾æZ=@ œ"†Z"?þ$àŠó?ȦˆÂÔ?™µ÷ü®ðL?Ô|Š_iòã?ü¼xÁ²½?ïüÿ?:Óf?Òß<ã[/¿à¢»ìª¸¦¿à. ÿÿÕ
¿áÃ_eÁ$ù¿×m\D#›fAGNbll1RXS J095508.2+355054?ï© Uz?‰ðÌöRql?Af6^÷ç?=–:aèÛ²?"£qû0Ä?‰³b»fü?ï]fmZ?–ä
ly×
?]¯æ3žãÖ?gG§ä´Œ?›Ù_¯øft?–%I¯ì?íàv-âÏ?'àûz¨.È?z­")'õ¸?p%IÞpÞ?®¢êɏtS?'–K!¦4?íÙ	Ýt*?"ØŒþ&t?ŽM°?}¬Û­S'©?ªÜè<»Ü?'»¹÷²u4FGL J0955.2+0835¿äÑÔX²H½@F=ã!¢ç÷À;Fiž)KSÀ<™§ågÎ@D‡Åܙ@ø¢×/ý?Õ@'&5t?³Ä»[`Mó?Û£VœCíì@4§®/RÔ¿ç=:¾Aê|+"Ù@y¿ç0iTWp)¿Ò¦^äfòR¿æuÌ}ɯ¿ïò›]¾÷øAGNbllNVSS J095501+083342?ïTZÌf]8?B$yç™ì?U"—ôƒ¼ú?PCwVá?"\óì
?ŒhÖ¥© ?ïDمô®??';"U÷Ì?Nt±¬‹ç?W‹ÇHÝ9Y?–pS›ÜÓ³?'¶DoeÿŒ?îÀ~}A?€ÓÌgCÎ?zÀãs j™?j©‰¹YŸÄ?«;«‰´€?ŽP¼ÄŽà?î÷Ò•äœ?ƒ
ÈHFç?Zð´dê0Ê?N¸ x5?ŸV³&ôÉb?'uB‡û¦4FGL J0956.0+3936?îÿÿƎ0@IÞ<âž4À:ñù²%hÀ<½>Õ'å@`ÕwuW@Ò7y…?Å
½]Äu?ªéLŠGA2?á…Ñqw<?ý"È<V?î™Ä%^¿Ö‹_ú¼t:¿èŸœb¡µÈ¿ãV:Ÿ8?¿áBUå墇¿ïÿú Âî'AGNfsrqWISE J095608.57+393515.8?ï±ev£Ôð?tõ•
ÙsO?WŽ»ƒB?P>ræq?€´ßtSS™?sZLÔB´
?îõŽøOIt?–m 'ˆ´d?c­ÀÍÕ?lÍDÿÉt?žØ€Ýý÷?"¨Ve´h?í³@o,`³?"½!1Ïå?‹Ǧè{?fÃ7¸?®#ÕÜ?G—?îF³sÓ¿®?Œ…Ë~¶`?—$ŽâÐgÅ?'mK?
¯? Q[ÑE?ƒæ© ³–*4FGL J0956.5-0958¿ï«.y5@@ÖÌ¢Ûa»À;‡þzÄÂ<À<¿Ã€ó°f@!ªpI¿Í?õ^x%«‹4?ÞH×à&?Ød¡ŸøXl?úª(Èv%÷@Æ+rõk¿ïúŒ"¸'¬?ïÙû¿(Ÿ[¿çã4å2t¿½‡âž+ŠÙ¿ÜNczΨD¿È§^hÁ	 AGNbll1RXS J095627.2-095720?ï¸èØ°m}?z1ºëû$Ü?VjmW7š?Tˆæ2yob?}ðøQû€ƒ?w"°[?dÞ?ï<svõC?›~ÙcÇ<£?a°x¶9?xYƅ!~]?–;0*s?–ÈR ¨i?í{$ÌՂ#?—S"Ñ©ž?…_᪭p ?vúYä
?±zÝcþ@à?" &¾](?í€`;YZ?˜QTÍqRu?`Ìö†'å?aÄäå4ä?³v–s¸¬K?˜x²†Ù•4FGL J0956.7+2516¿ÓÖцM•@IzÒ4ëšÀ9FÁ*ØßÀ<Fx*´±@zŸÉ3%@ç	#•0~?­PLž"*?¸cÐ^ý'f@~5Å´ª—@0ïŒv¿Ðû"‰µ ¿ä¤
ájÿçb)Àê¿èû¶ßû}º¿í¼{Eñ¿ïúàSG%AGNfsrq3FGL J0956.6+2515OK 290?ïÖ¦GÅ?rvquQû?PÙÜ{›?JMJÖpqí?p¬‰*?p«baÀ™Û?ï/GùóL?™êÚD.¥?fV…þˆ×?€c%‰]È?—L0Åbr?•€w˜Œ,q?ïàßø©?'æŸÌ»%?t#7"IB?bpmÑ
[D?–û9ÉÍ7?€~p™^uú?ïž{ÆéÃx?r—Á.IŠ5?zï3Oj½?jŸ1À?uÒé;³‡•?cøvÊgú64FGL J0957.3-1348?ïq¨ºÚî	@?.+{®ÍÀ9¦©ÑAåÀ<*ø; ‡@SŽºB†@zÕٻș?¶r ®Ì1?Ãà:±@0
ÚN•@úÓ>«âG¿Ëƒw™?¿á†"S¼ì¿äŽ4 C€¿èqéòwA¿í$ŒVºø¿ï髕D CAGNfsrq3FGL J0957.5-1351PMN J0957-1350?ï¼@¬>Œ?yÕˆ?eN} h?b-"'´È?w8k^iÞ?t$ii›z?ï¢-§œîi?ƒ†îÍsh~?L½·ûVp?^˜ŒX9É8?…¨Ä½D°V?Ÿ%3
1x?îiÂBÇ-B?"
"þz­•?ÈÉýôÖ?"3£Tô‰?¡q×!
®"?‰ô—ÏÏܾ?ïÈçá !M?aΝýVŸ¦?\z:"»ø4?Iyƒ­,à¶?tm€ŠÀ[S?]#£éjŒQ4FGL J0957.6+5523?¬‡Yk¥AM@G÷7âÅ\–À7Ìo¯»DÀ;+Šƒ|!@º	^" ?þgbzH›z?ŠñnÝ`÷?´
š7Ï$@@%Áã†Lµ»@
%@톿±ªà=íÌL¿ØběOý¿à•OB2"¿à[
bY'l¿äS¡2OB¿åTWp)]ÇAGNfsrq3FGL J0957.6+55234C +55.17?îíJjT®?®îÜHgê?hæ%!q§0?iG‹Âb?Ÿ9îOÕc?œ%2¯Þ©?áxՇÔõ?ÚhÃhç™?Ùg*ŽÍ?Ú+‰ñ<CU?±ïã"&?°æº²8@
?ê;ÐDª/à?®ÎRˆSšÀ?³)ЏOô?¢úÞÑC
?»T
1?§?
¿I…Ý?ÔFþ"û+s?¹ÓŸ6ö?Ùf'u¸åI?ÁKü¹ÓFÏ?ÒRÙõKïC?¸Óá•%Ðä4FGL J0957.8+3423¿ç»£…¼Ô@J&îcŠ	À:t¥×ÛÀ<®!õô
ƒ@)ÒÉ*@q<%J<d?À–%›Åî·?ĸØú¹>@(C(†@Ž e¨"?ïû›¢|K¿ÜqÎäÕO¿ábTŽ†@¿âWÝ6§[ú¿ç¾RúÉ¿ïöCôK–×AGNbcuB2 0954+34?ï˔)¯i?u·'oCí?b¾æ3JrA?dÖ¿7Î?pÖx¦C:?kÌ»Ïæù?ïYš}n%Ø?Z¬ë$ðË?ZGãh?g^}7åo?"(7€Ý‰?Œö瞈
 ?îô"(6Ø?…¿T׍îñ?xúM˜d›j?s¯†qÖk¸?›0癿þ?€²‰XÁ+?îð""Ã&?€§¶–9¼ø?†ìֆÖ?kø'qgå†?–‰")ü™o?{Õcî™õ´4FGL J0958.0+4728?íþÉLmI@IU·|¯ÞÀ9›"²ÈÀ<1Ø2[@¿B4Íg@ì&ÿ½?²SõuuÊ?Ð?½t•@ge47?1@ùnõG¤?Ìÿ‡	I)ë¿Þ²…³¹€¿éTÀ¡›EÁ¿ç‡»JÄIq¿îíŒàΌk¿ïÿ "_õAGNfsrq3FGL J0957.4+4728OK 492?íågÜ«OÀ?¨Ôµ·Qf?«2öW›?¤Ñänô¹×?‰Ú/v¿Çô?'"}pòmh?ï\È0{ý?"Χ$Ñ?a
UHå¶?t$%TJ?']¼PÓÜp?'YçÎëʆ?êÔ?ޜ?°¹‰€»*¬?º(/‹_€?§ÃA•;"–?µQ.¥?¡ƒuZÈ?H*?g[ta¯pZ?jԞp'?\-o–Ñg?q€Ri£åª?^=9Ãd4FGL J0958.0-0319¿ïOÛÎ%@C%? §?À;œ¥ŸaY·À<Ê]Óð­}@"˜ÕV‰#«?à•<<Ç0¬?ï6jXŠÜ?é±e¾àÆ?üõÅêZ|@²Òû¿ïýcm¢?eÆ-¿ÖUGZ1¥¿í€ãŸø†?ê·ãÑ̿⨈ŸÌ8¨AGNbll3FGL J0958.3-03181RXS J095806.4-031729?î=­ð¦iæ?­5>ì"¹ÿ?±Ô9õ6?'Ož9±9?¤8«ç Ô?ªgǃ.I?íï'mÄ3N?¹uå1«-?±aJG^o?™HMVÃk?¬¡0Ñ*ó?·@9™¤Mi?ëN–Ø0.??¥â1uˆ™E?£ÝoWê?'¸ÎW7?¼Z°Fâ?£:ëYl O?웻 5‡ï?±Bi˜Ù*?$`¼oҘ?PÔnq:Œ?»ö @$?±DyiæÇD4FGL J0958.0+3222?ëyYnl€@J!æî·`À:oÎ=UÀ<A©î{s@{k™¬@Ý«ýIl[?¼u_þmXÉ?°ç1ýÔÉ?ðmjœV|@"ëa¸W?í™j4Q@d¿ç@6¡|¼ê¿çE\á,€<¿æLs@i|›¿ë—¬ÂkJ¿ïõ´¢‰'JAGNfsrq3C 232?ï2[àî©Q?'$EÍbþV?…2C[<H6?Î6G°Ö‰?Ž6Äic›?‹}òšÞ¯?î´m͘?í†‹Ï¦Ñ?uÑÜVO?ƒGÕ°Ü?¡ÿ÷£³
?˜WlhQZ?í—Lªx«ý?"¤ÁÉ¡ŠÇ?	Ê=?'´É Ë2?®C0Ր0"?uüG(?î@õää.§?¿˧X?¢Žž›ž˜]?ŽËӓ?'Ä,<ú?w¾ÝÔkË4FGL J0958.1-6753?ЅîvÀ¦¤À$™ë…¸RÀ:ö•mºîÀ<C¾˜V£{@始ʣþ@ùPá™ãk?¿Yô›¿´B¾$=w?÷­N·ó÷´@Y±rµÕ?Ԓ{'­Cð¿ä¿ð{'¾‹¿èH4rß¿áŸÿ¿"SY¿å´ÊAؤ?œñ(™À'AGNbcu3FGL J0958.4-67521RXS J095812.8-675241?êõ]hü}?»˜íØ)ˆæ?{'N둅°?pÊõ"	"?Ç ÿß?»7Üô
ð?æb•LO·?ÈMëêPN?kGSuƒ™?vÛ†ÿÍ?Ӓ¬/bu?È)ûÆÕEa?ëˆ/-°A)?¢ëՆ3ç?†zvö‰lÙ?qcï3)•Î?Àw›ÙÖdŠ?¡œìfýƒ#?ëlõët¤ ?£!]z‰%?|;¡š^"¾?pèç^L™´?ÁjKEZ|l?£«*¤Q4FGL J0958.3-2656¿à˜›± @5Éó×ӑÀ;EeÄ÷1À<ª%s@-ÑRB˜?ÿùI²Ñy?Óû¥ˆ€?ÎrW`dÙ?üX(&·@õ^'?¦ÏF_ñéM¿Æƒ¨9¶°¿ÑߥA˜{·¿ßƒÄKžå¿æ8ßå®E"¿ïý²èõø?AGNrdgNGC 3078?î^—DÖô´?£¯0±HÎÄ?‡¾9Ï܃á?…®!L¥?¤&ý>™"È?¡ÖËÕñ?î¾V©›?¤3"qñÞÈ?Vû•HíU?"¸†Ë3$?«X•5C*ý?¡Þ•œ	ƒ"?í*åhƒ³·?›;,''?"¨ìU8fÍ?‡ô®EK?±¾™¦"H"?•)ì'V
?ëU
ä2ã?˜£Bè,£a?'0eí@Ú²?{oðbº'?À…DZŒX§?˜AØ´ór4FGL J0958.4+5042¿Ë_ËñÊL@HâãK"SÀ:bŸ1‰À<²Š¬–Ì`@iÂp}k'@ûµ¤at?¾ª ¹.Æ?­s\f³=?ê×'[å@
ڧ옚?â<x¡|g¿äÿïÕ¿ço˜p"¿èàíìEz¿ëèߥ¥¿ðAGNfsrq7C 0955+5054?ïày70´Ú?l8ÊñÉÿ?TԘ†tXH?NŽ\ÔdŠ?e|Œù[?g'ęJ«?ïs¬ÿ'~ð?µh­?U{ žÕU›?gf²¼O,
?2¦ÂÌÐ?‹òý4׌)?ïLD³ö?†-"BeYñ?p¼˜Œ°4J?c0 ?™‡WÔ=t?"b3E' š?ïš3ZÔöE?pAcªÔh?y?_H̵›?dè6«‹e?y¦óL¸(5?cÚxJy4FGL J0958.4-2441¿êè
yfÚf@7|#̍ãÀ:rçy }NÀ<WË/=Û-@º+Kˆ?@	`Z³«?Áw÷ˆàd?É øžï"@È9À.e@)Ï/þuf?ÓÏ6JÀ¿ÛQc'A¸¿ÞÓA:ÝÌy¿âQ(Fp&Ú¿çñðÃL¿ðAGNbcu3FGL J0958.6-2447TXS 0956-244?ìÁ2ëlïŠ?±ö2'™Ó?¦.£x >‰?¦zûôôx7?­¾-ÑÈÆ?¤"wYˆ&Ž?î½þÛ[À?¦êûM??"^Ïsý©¿?†¬u"éV?©ll5JÙ®?¤4¢ùd7Ò?ì#>O-I¥?¤°CÓx­›?¥û·nx?™ÿ'Þ:±?³è1ϕvÚ?˜KHi¤]j?ë1pcb?˜púÒQ€¬?š©úïò¨?€¢±5?e?¿Ê(îÐ?–0jåÑB4FGL J0958.7+6534?ÕAlÓ#9Q@EYtæ[êÀ8rÐ4³À;´~d‰íT@êƒ-±@Kv Í|?"åL"C>?¢ÿPËN@BåۑŒ@¦±['1É¿·(ÃÂ>~¿àåÜhKBô¿ãƒÿiKZ¿âýò^¬³¨¿æz¿^z3οᘼúDZÛAGNBLL3FGL J0958.6+6534S4 0954+65?ï´Øø#Ï'?ƒ´TìR"?CTY ´?GÈˇš5_?˜¬±z*Ô?'¥ÂäiN?ïzê"?•ïãømYž?Nó7cÖøå?`ÕÂp&?ó?V+'oþ?•"˜Gµ0U?ï#¬¥Â
K?"KóÚDeP?rr&yË?hV½Ñ­{ð?–ã&k4¸?'YÍ1 =?ïþ«'K8?²ÚԈw˜>ñGèu%B9>ê"OîL
î?#%À|§Â£?W÷œIŠ4FGL J0958.8+7039¿×ÄC¹	ÃÆ@D$ p¹À;Çp‹ÔÀ=%Æc&@@!í³/³ø?øÿ&¡Txþ?×ÚQðœ5?Ñ${tëdh?÷ ªêúµ=@ߘ¬^ÿѪN½Ó4Æ?Ö{4©«?áÝhã³?³àΌj‡¿çP䉁ôa¿Ì.îúâ	AGNbcuGB6 J0958+7039?îÞàÅüâ6?–|m(€¢?kž'e'¿?aY «:? X
‰ßl€?•=#ǐ¸B?ï?Ï©¸«?•dÚH¦?^-Êø½i?l…kr‰9b?–;.^Á?",ˆ/h?í(˶ø.É?š97Þ@É?ˆâoÁÛO(?|ø­Ê¦*å?³TPÌ?—jq'a¼Î?îs"9ÖWÔ?/'O˜@D?u~=ƒöh?k·pÝ5S?¦ô¿êÝ?Lˆ•4FGL J0959.4+2120¿Ô`¶ y¯@IH8Ÿƒ¾fÀ:§]u&ÊÀ<…='[·@€Ù% £y@"NCYñä?Àªa½à濋—/Üçw?Éü»§áZù@gNåúÆ¿ˆ@ïÎs¿ßpš1o
Õ¿áéžÊ[…¿ãgS–€	¦¿ß†3‹GÇ?¿á¹ASAGNbll3FGL J0959.7+2124RX J0959.4+2123?G,¶ ?¤×UĪF?n
K¤¢õß?a
2y`±?¤ã¶ÒêfÀ?¤[€O+êÆ?ïˆØ÷*?…"™¬Ã-?EûHCtY?T†^Äæ£?Œj#þÞ
?ƒÜr9/8?î0RxdE`?¶!¯&u?z·à¿?iÌfœ »?©£Üx¸2,?Œ™U^Žçœ?ïuoø?|M~m¥E%?kˆ#ÈaG'?Vgôý¸×?™€[xôÇ?{ÝSsg*w4FGL J0959.6+4606¿æ­VBŠr@I¤¹#¢œxÀ:¾=¢ø½ìÀ<u¾{Ñ1¶@$›7(‹:@Róš–ï›?Â×ø…bU¿¤E_@éep?ÚµgÀÙyƒ@=Ò™™?Ú/é(M&¿á­ïýS}V¿ê^ç$.³¿èP"Xð\¿ïÿòÿf}
?ïr·bWcAGNbcu2MASX J09591976+4603515?ï§!| @?­ï±(?tknãzð
?vß(HÀMó?xÒÌeÇ?­äÉ$iU_?í³Û²<ƒ?­'àKŒí?"Í!'.3Ã?êðÞxÇ?¯Žüw³ºþ?©"{Ô?íO¬Æúº?"{¯dO³?'#8ÆÚ ?ÌJ'Õ$?±9Ù³–s£?ùÛGü}8?î^{Ì
Ø??'+hAÌ?•'b¸?…†º:è©?žŸp@òZ?‰‡]öc'¬4FGL J1001.1+2911?›ËjՔz)@JOKrÅzÀ9z¿ª¥Z˜À<^×,¢z@wÐ1[AÅ@ä#¾K)Ê?«ÉªƒvÂ?®éO[Õ5I?þ¬5}N—@kd°-Û?ÁZê‡GÝd¿áÜ,¼ ­¿ä¾ýÝ;¿äÍi_•ô¿ã˜†t"è¿ß¹ö{œÙjAGNbll3FGL J1001.0+2913GB6 J1001+2911?ï" %²?…¤ŒVY?E—^†S©?;&ÿ'ht ?‰ãÂÔn?"Ƭ•Çrj?ï§5È<e?"´èªžÐ?AH¸Lߋ?Q¬§ËJçŒ?…l%K?ƒÌ¢ìÚª6?ï­ÖÙD?ö½*³`?l‰˜¸su©?[ᧄ™Áˆ?™N7.hÛ?€e[½A§	?ïõÄhÉl?B*u @?1Sikh"? Êñ*O?P"mRÍí?@Dø'%¬‹4FGL J1002.5+2215¿ïwð7¸ö@IÂ/¾3¬ÖÀ:Œ¬nˆs×À<wXï…^y@ žv{‡_Û?ýä(3$ðz?Å‹ypYY?›˜+§Åù–?،üÓ$Õ¢?ðÆ+«T'
¿Úם‡ý¿è
ÀGƒLP¿ä.]
¿Ô"ãQs¿áƒ÷ÜEÕ¿ÕÝÖÿžAGNbll3FGL J1002.3+22201RXS J100235.8+221609?ï:mYÁ<}?7šqë?S£ÀF.©W?Ktx`&s?—xÃu…©?ŽX¨ ²µ?ís¤7B¡?³>P.Ù?K¸l²`ö?šØý'EÈÀ?³±tÃRÅ?°S§&Œ¦ç?í¨ÀÕͨc?"¹`Ñ­,?~)–4¸‰ý?q¬üß?°×_îG4A?'廈Þ7Õ?åÃ|̅àl?­
"'2½{?¨q9–¹!?"WÜÌá?Ñjß4d?­VéHz™4FGL J1002.8+2140¿Ûï›¥Ã@I³ÌcñA À;c$W@YÀ<ÂWþė@ÖZÖæ+C@˜ûyˆ'?ÊôµÉû⿦³vºq€v?Ùy3]$žE@‹ž†é=ǿ什ÿT‰o?îE¶Ãvö¿é=1ïfTÉ¿ÒUUM9¿ïªøÎÞ?åo‡wX&2AGNbcuNVSS J100250+214225?íÉâ½TùŽ?¬|և~?u––ô$®6?r
ìXeù¿?°W€¦è©?«Íß×·à¯?ïz³Y+¦?•tQÏð8¡?Ieõñvš?W´v¦óF?¼ÊKåþõ?"úϑ[°?ín]U/?œ™9d"I?ˆ‹KF
Ñ?{t§êöƒ³?´c&ŒS5.?™ž
 a05?ï)ÑÊö4?"&»ªÒ"?n¯ƒ~åq?cn¤¨G•¨?—°Ì<Ì?''?3bF4FGL J1003.4+0205?Õâhm°:N@ESøüÖÔÀ;9|"NÀ<¬#þ	ù@Óy³J?ÿpŽ•·?È´ E°8m?°Ü_çÇ$?å•ò`L–?ÿµ³–??ïî"%âؿꐀýÁ?³$œ—zÛh¿è¢JBCqo¿Ú¹#ã	$A¿‡.tɉ)AGNbcuSDSS J100326.63+020455.6?íé+S6eš?¤8øáԇ?^ÕDp2Çë?S9tPã?°;PTŒ?¤oçTr?îÜòyò?¡"Âq ù¬?jÝÌ/ÿ'­?r…]xí&@?¥bmØgÑ? 
É&¢?킺UÇÇå?•ò­t´Ë$?|Ô±¾¢ Ë?kc3×ò^
?²â5זÍ?"ÏÒ&Žž?íkxæ÷v?–oRÉáCÆ?wܳ62™?oK!ôroW?³&mC©'?•Ö­-«ˆZ4FGL J1003.6-2137?Ð-4‡Ï @:ÐEþÀ;ŒŽ·¾HÀ<À
(ÝnÛ@"ÿ2ûé?ùú5 Ë½?Õ¦_»&‡(?ÀJ
MzÝ?ëbC¡ÀY¢@#fón¢¿éaßî聿é/"þ)f+?ï:Î2'šy¿Ø7±G5H·¿Ø5H Öj¿×A¼ã˖íAGNbcu1RXS J100342.0-213752?ïM®h8€Ì?Ï–ð1£…?A&5i´J"?<¼-…0œÕ?•ÁM¢Cþ?ˆ †Åj?ïBA{÷jÉ?› —pl?T°"?ÖhÂ?f\Qø·ó?–lÇM@a?™ª¶À°a™?íÊð܈Ó?•ÖÿԘ;?jn³ìñÁ?S©KWnvÜ?°Õ|QÞÁ?•ly&ê;?î©ûž©c?Mþ¡ã?>¦²Õ(òÿ??ÀáÜ¥!T?¥"ø¯Å§æ?ŽçWÏ°¥á4FGL J1003.6+2605¿ìMdø'C'@JTX`fÀ:›k¯{ƒ.À<wú ø@
?h ¨W@"¿'a?Äð!e«U"?Â3£Æn8î?÷O­¢e6?þš<â(¿ë{L§xn¿Ù2ñ#Ä*g¿ãrZ?çvœ¿ç[§J¿àÑ۔æ¬r¿ïüfM;òõAGNbll3FGL J1003.6+2608PKS 1000+26?íë‡×)H8?£MÅåH™?|IÐ4Çí}?t-…cÚÃ?­¾H†Ò~Ô?¢Qx<dU?í±Ïq´]ê?ªÚlÎ/{?ƒFå³i¡?‰ù†+³$?°§»ïï¡?§ÿ'‹ûX?íwï.J?•2§"îÙI?ŒÜ*È0Ö?zw	ï£Ê?°¥4©ÖË?'˜t3Ê?ëô"0Ds?œÈÓ¿7C`? §Õ×҉Ï?Œ|~îvP«?¸ó"$—ˆ?˜Î>62jú4FGL J1006.5+6440¿¨Á°õ6ë}@F&¯%;À;*.XØß*À<ç3cښì@ ÷êÃز^@©}'Ô?ºrzù*¤¿¿Õ€r'?òXåªda?ÿã­¹â}¿íÐQò;_¿á½c£=‡¿â\ᢜ́¿ÖGKCdt¿ä	Úÿë]1¿²zs8±ÍBAGNbllRX J1006.1+6440?ïMA¸ïlL?®š™?ID?dÆþ¯'\?asãZÜ?"Õ<"}?®yž;?îð…ÓÍçá?²![ÅÖ?dÀת.Ð?p$í†Þ[?ŸW*¢½ò?šïCÿJ?î*.tfè?h´Æ %?uü>æô¯?lè&.‹?ª—&œ²á?Ž]ÏVh:F?í|ÚúÕ??'%RÄ
ê?Ð._¤W?úíÇ"?¯Ê9"Ùãæ?ž¨oÝI4FGL J1006.7-2159¿â›6®¬•@:Æm½r¼¶À8aKŸŠÀ;ÊÊ·H×	@ê'1È$@ZaÎQ1?±!ð@+?§Œ%'¶¦p@хÞz@¿´Û>˜¿ÂŠºX«è§¿â}Wyc™-¿æ8"œ×%¿äÙ>ö
¿äìÉA|÷ø¿èw]š
_AGNfsrq3FGL J1006.7-2159PKS 1004-217?ïŠi)"eB? ˆÂ:6?H¸ï"Â¥?W³k-Iö?‹Ú5{ísX?ŸÎIìhÎæ?ï²p9-ï?Ž"é¢É?A
²$9b?Vsæ¤çÂ	?'SF'CôŽ?ï?ïAÑ«S7?…'éµÒdh?mÖü"åÎ?ZÖ:‰ŠÛ?˜†
ëüO?"üüY?ïþ8
e©ª?!5—b¸-,>ð¹
ئ:>좱ë©õ-?*h7êPˆ|? k…î´Ó74FGL J1007.0+3455?£Ïò;Q½@Kà?pÀ:š¯_Ô{îÀ<Š®¬Ÿ0@ oè;=B×?úùcc|§?Ã#öiÔ/?Á*¢jùs@Òz{Ç!@g&q÷?ïÕřҤ}¿â†ôæÇIÖ¿ËåÛf˜Z¿Ôñ§ãxu¿à ÇuË¿ÞE`Ý:ƒAGNbll3FGL J1006.7+3453EXO 1004.0+3509?îçéÀ+à?•t)Õ,È?m?µœ4>'?dËt½R?ŸZÑ:sü5?"sŽ¶¦?îРô'.™?™Ž6ÐÌgÇ?kïҝŠ?r]=u­ð¥?¡EÀc=Ì?—†ï¶ÿR?íÊnFÏ2?"6p¡Ly?z÷' Ò?e/MCô*?¯ú+Pmh¼?'Ã
]Ÿ7?ì)÷¶—?–="´-d?"	Š®Îå?zҝÿߤ×?»Tô¿‹?•fþ7;j4FGL J1007.6-3332¿å
"4Ïã@1õßeUÅÀ92 
¼À;ûN']Šö@¶‹¤ô@<ï>çœ\?­ý"ÀÁќ?Éü§ZøI'@ÿõbLM@÷Æ0{s?Юý®ìè¿ÞÁ {öpŠ¿ær¡Þ¹¿èkˆVÚØ¿éÄP'èË0¿ïÿÀtϵµAGNfsrq3FGL J1007.4-3334PKS 1005-333?î<‡®r?¦ü
˜¯BO?¤¢ûÒP—Ÿ?¡w6RçÚÝ?–f`Êiƒ?– ¥Úh
€?ïm¬{ßÎé?–ÅßÏ]?\8øw 1D?lé¸SÛ½®?†àü"Ä?–
ð©äu?ëæ§L"ì¹?ªòlÁÅø«?¬‡²Vje?·®"h?²†ìp+–?£þJœò"-?"µöc?rê6¤2Šê?iècnêQ?Zýk©ù?"Êàù¦¬í?n×»Ñò4FGL J1008.0+0620?ß,˜ú¸B|@G×süÀ9*¼ª?ÚÀ<¼ bv@Ù'ÌLÊ3@B+{®Í?«0ªþ×ó?¨)Ûúë?ü´d¬R@ºË…$?ïþ[à¦sr¿ÎBßN"¿ãíÔï°ýc¿ãˆ¿V"¿àºÇ犾5¿èZ€êv+AGNbll3FGL J1007.9+0621MG1 J100800+0621?ï¾!™§"?"ª;Y9r?<
¯ù±ÙÂ?V\ne+Ґ?.Xzj?"pÞK¤0ò?ïF,'õL?ˆ$<óCî(?GםԐ?V¬žÃ€.Û?Š°û¹« ?†õ+¯"š™?îíð:^ð?…í‹Œ`a?s'íÇ°é"?gã­(ùC…?]}M§çƒ?ƒžÍ‡ÉÁ?ï¼¥Ó]Ú8?eö½´U€©?c2A"+½>?Pþ>~á¡?xõ‡}5?b"xð_­4FGL J1008.0+0028?¹L	Cbº¼@EO'j@À:O{ûùáÀ<n,·/¢@1¡&@&býüÁ?Ì-µÅÊ$?»¢""EA©?÷'!A™'"@Y ­ ?ïÿü¥¬¨¿à"ßq?¿â&±$ÿà4ÚÓÍ%¿êø×ý­j\¿ïÿ‰XAGNbcu3FGL J1007.8+0026PKS 1005+007?î"%»µÊö?œå8uÖg?uϨ#†ê?o=0ˆŸ'<?¥êOžßÎ?›]X¤_¬?îè"©ŒÚ?˜Ý $ê0?o¥!Ȳ?{†"»—Oº?Ÿ
&•N'?•ÌXÉLÅ?쏻l¥a?K²s N?˜ç«:"àº?‹Gáú?µMçUõÜÇ?•ßs ¯A?ìì£ë‰‹°?'ƒ¦y2
/?£
É4
*?…%ös³`?®'øZ0Ì?‰áÂ4FGL J1008.1+4706?ïÁœ}¿ì@J4ÿëJwÀ<	zP(6€À=!iθ@"tRBÂó/?ÕÑȽ/v?ãj@ºˆ'?ï
{é…j@1¤Òh@|<yX¦?ît#=qÐ}¿ïÿúÁҝÇ?ïÿÒ†ëA¿Ü9™aܔ?Çaû'©¿é- qäAGNbllRX J1008.1+4705?ê݉ž#3?ÇZ$aêœ?Ããèmq?Œ|DÄ?Ãm¨‹Hì`?ÆÏ"SIÎî?î.^Üsõ?³ö
wÉF?}ÇÆͅ©Ê?"´w¦k?©aHˆ‰?±ñí{Oï?êhȶ>Î?®àž«eG?'{hAƒã?ˆm½…Ø?Ä
p×(c?®Z·a²?íNn™ÿ?©í6Ž÷?3WZ˜e¬ö?=Ñ'Àxl¥?µy3Ü¡Ì?©ç‡jW24FGL J1008.7-2909?Ð:3¾°@5ŽÊW§†ÂÀ:Œ½½eP½À<ZTtÌZ·@qgd"(@ic¦˜…?È
£‡"S?̦C̪ï@€†
 z@
Wr,Ã,?ïÿÄ}îB¿å«fJ¸¿æ'F–½FG¿ä‡`F'´É¿ïý.>Åè¿îŠøìæGÈAGNbcu3FGL J1008.9-2910PMN J1008-2912?ïšû?Åš?ƒ˜y>Y}?nø,óZ×?mò¼ý"ø×?ƒ%ÂÂÀ?}¡ëIå¾ê?îŸñÎÂ9Ë?Ÿ¹¹Òk?€kx!¨J?ˆU=Àê˜?¡ær[n?™³³÷¸­?íÒNÙUç?"ÅìÀ):z?'8âÔD	R?ƒsn`,¶?ª>¡…ü×?PxÄ©™?íD9üaÓ³?'úN·ôÆ?È>þO?ÐL
"90?¬Ø@ùãÁ­?zH¬%4FGL J1008.8-3139¿ï"ÿ	F6@3˜>BZîcÀ:ç6žËÀ<•ohm¨@.tûª…Ð@^ܙÉjB?¹ÝâHßí¼?¦/³Ýù¬?íF¤>¹#M@Tóe轿âÖ÷ÞshX¿ä>Sü×W¿ã/c?•l8¿åú,hJl¿àlk΅3±¿êº¯"ÖáúAGNbll3FGL J1009.0-3137PKS 1006-313?í"@^¨ëe?º¿9'ûTW?.ŒTûÿÄ?‡ØՌ±?±8+€$Û?¸D´Ä*?ï+x$.%?'
qw‡k?_^†QÎ?eɦ"²s?˜›}6]?'%ð\çÒ?ì¹'wòâ?œ'}cÙ?'¨¤CL?€Á?•^ß?µ°Yà ˜ ?˜>"ÛªÜ?íCp5˜ã¾?"€.ª?ƒŠMòùêŒ?o¿åt­
?³s4"Ù¤Ä?'ÁqqÝP4FGL J1010.2-3119¿ï²	Š‡@4äy'¼À9"pæòèÀÀ;úio/bÄ@!PC÷¦•+?ûã#·;k?²'rásøË?'ÒóYçl?â3òí†+@
!"}ö¥ä?ÁrI«7?²L'S$¿åŠÛá<ÆZ¿®æ¤ o¿ä¦],+6¿Àf‹û r;AGNbll3FGL J1010.2-31201RXS J101015.9-311909?ïæ®gáB«?d¬"…‰BL?._™Ï×?"ªc?gkžÃ"<?d šÄy¢?ï³Ð¡o€Ë?ƒ=¶vŸ>L?Cˆæcñ?Z»aÁ¤ ?ÓI=ï\å?Ë(@xù?îrW'1?•KG+'Ñ?n0qÖOô?cÈt¥—?¦÷Á÷?"ä<0úµ«?î™l쁥*?Œr7˜a"D?q7ÝȦb?bB7¥áx?¤HÊ<,˜?ŠãH ãw4FGL J1010.8-0158¿³ú'^žÙ»@DÍæÿ}úÀ:$<ù…'À<UäíU@q"–ØÊ@gÅá÷?»ÌBŽDü´?§M༠ŠÃ?è®~F¬ã@	–­…èÝ?îþê÷Z?¿æxK5ˆx	¿æ'bO*‹¿ãqYßofÀ¿ïýé:ø$¿ï4v"±ÓLAGNfsrq3FGL J1010.8-0158PKS 1008-01?ïÀ¨X1Kq?'¼ ì1äO?`žæ–ûAI?Y–õˆ?w\`›Ü¦¬?'<$ bD?ïg³qjö>?"Üq"p‹?Y6©'™Aµ?q_¦eZ?'v':w¤?'-=#9K‹?ï#è։0z?œvøñ¶?s0׃#
µ?cפYYÜÛ?–¶¯N.?{Š—ȱß?ï	·&p#h?€¤ŸÞ|2Ò?ŠiôÈ!)?v08\›:?'" Íëï?t4ˆ³}j4FGL J1011.3-0427?âôî´©Œ@D
êÈ`V'À;R%fÁÖÀ<y_×Öì
@£òž­œ@Òÿ#a.?Õ&¯aû?ÓFÚÕùò?ü¶¡|¼ê@
™«Ã<Ö¿×w؞è
¿å9£ûkq¿æ€Éë£R¿åo쌅´à¿ïýÕ{Zi¿éÏ
í6ÐAGNfsrqPKS B1008-041?ï:ócTš÷?'p+©¹ïö?g=gÌXk?alìºn®á?•¹æ²s?'—·mïê?ïæBÃ- ?šƒæêUpµ?bGÅÀpî?q^¡]]†ë?šz>ï˜=À?—ñnjñÖ¿?íz>òz?—ö™éWl?'®«ì7Æô?
¬
ð.Õ?¯"Á*ÂDÒ?"çÀqq?ï$™}v0?°º™1ß?hµ©›ÑÒ?ZXÒ¨Ñ?˜V-‰ª?}U#S˜s4FGL J1011.6+3600?íL*R¹á8@KŠ($xÀ;%t…
À<Ú\ђ.k@)©m¢ñ@"õÞ>Y?Ë|¢¨a­?ÍwY}ʱ@A@š$?÷KêlQ¸¿ßC\¡¹Ñ?ïȯÑêBÿ¿ßG.<ÔF¿¿ç™mYŸ®‡¿áó:u¿ïþ®üØ-SAGNbllNVSS J101147+360019?îë^(†c
?˜³ÒÙx²?PóWj°t?|nü‡rš?™ëÁC~F'?•˜ƒÐ=Í?쀘|3_??´…Sð`?¡Å*PœPo?©bó³­?³¦öÝÙ?¦ëýÙäS+?ì<àviKL?¡úì*HªÖ?¢¹¨ îV?"¦É
?´¼(<³®s?™ôÑÃ7É?ê¯OH{D?©1‰b¤î?¼51"rl\?¨/ÀC­?³½SòI¹ˆ?šÆ™0g/s4FGL J1012.3-1232¿ãâ¦[|†@ARÒ^Ý)À:Ž-–;@HÀ<Rv'=\'@̀½)Áš@l dŽõÒ?Àƒ­Éý9§¿¢ûä"ºü&?á Ÿiè&@˜&+ô¿"Ów¤É›¿éÓïk]F,¿çç	Ĥà¿æ¿¸èz0¿æ›}Ëú¿®04âF÷AGNbcuPKS B1009-123?îääç}'U?¢pìÏ»?'wՐe:?'X3Zv[?š'xH8&?ž«üþmÕÍ?ï²(vUE?"ÏáªÉ°™?aNœßR?iò	h?"¯?›ŸúnÁ»?'ÝùX€¨?í:ùô ó?"òkÒù³?ˆ[àÅ¡?wbüâï?°úĔY»?'~{5^N?îék¢Þë?'ëÏ/‹ÛÎ?ufä
©z?c¶&Ùì®?xÓI8v?6R¯{Ã4FGL J1012.3+0629¿ÃØT"*‹^@G~´À9v¹Ù«À;Ù;,ü¸M@ú£è'M?ÿ"~b®–?²äv6¾/?·åøÂÉé™@ëíœP-?@fŠŒ¶\H¿àÙCӔ¿ãsˆÃˆ€m¿Þæ×¥mã2¿á!‰¢«'¿áò] D-¬¿éçšät«AGNbll3FGL J1012.2+0631NRAO 350?ïŠúb9`?€VªŽ>Îó?^€š£úƒ'?SV{,ñ÷?‰qT9×7?~oeó—†?ïN§Üì>?"¼1ád?XätŠÐP–?gVê)#(?"œ½Ï3)?ŽcrŽ…Î?îûA¥ÝÓ]?†På€SÑ1?slÕdóa³?gI äc¼?›¼•ë»£?ƒ¯rŽ:ð™?íüzã&‹?—²€gPH?ƒanE?T[?lSÂõÃ?µ3î`>á?—zõ†>›ú4FGL J1012.7+4228?ᝒwë©@K4ohÜÀ:hÙÒnÍ=À<v½ôµ@ Žòµ¿•?ükWfï"?Àš<VÈ? A>â?á/WK@鄈»Oø?ïä]ý⎿æܬ1&é¿àö>"þ¿Ì¨µUⵗ¿áÍ)HÎ¥ë¿ØüŸxUÒAGNagn3FGL J1012.7+4229B3 1009+427?ï¼Õ'?ð»?tÚOs¦ê?C¡×Ø0cŸ?5""……h?!1e•5?sˆVB;'†?ï—9'#?ì?‡|!G??Eù"".dŸ?U·px36?ˆÒ5
>?†' µ¾Ý?î®9	|–P?‰€"Tì?i..be@?ZÍëá¤Z?£‰Œ†`t¡?ˆPÜñ#A?îðé؋W?ځ_ÜLä?p%zW'?ZÙ)1:"³?Ù™¦N?'?}ÍRfï:4FGL J1012.7+2439?í ¿jäzh@K0ñ€
|[À8¥î'):ŒÀ;ç(Ag©]@µÐÍbsé@ZA*2?¤.OÊkI?Á¼£´Ð'@æ<à[@aÓNq'?¡-àõ	¿àlh'î¿ãàoa6Ñ£¿æt -œñ=¿ì‡!œ1ú¿ïÿûÞ]BüAGNfsrq3FGL J1012.6+2439MG2 J101241+2439?ï`@™Þ3:?'ŠÉò*i»?…öå€kŽ?‡L4šGR?'êâ¢òÅê?…†šŠÖHQ?ï:c¥ª)?•¹R|Öv?cMªÖèœ?r,,IZ?–?óµïÝÅ?"[ʈ*œ?ìõ¬ã—(g?§"僣²Ú?©_‡÷¤èd?EZÏÓò?§E©Îè'"?Ÿ(J|U??ïÜtíh"3?_qù¼èßÎ?WDˆÅ÷™?L§ÇX|?gèÊÓ	Ò:?XŽ«7¤Ý¿4FGL J1013.3-2551?ïð¸Ú|Å@8Â÷ÓÀ:¬l){À<L-ë˕•@Œ	K¬Ò@'óUÎ?̚Ïú~¶¿?á=ö¬m²@ø"5´í³@eyœÞ?~[lƒr¿à×ϔþ)f¿èxQJuo¿î|?k¥À¿ïÿÿ" 5•?ïìÝxìzèAGNbcuPKS B1010-255?죦"Až?¶¼0Ȃ´?²Êø¹œ?²ïo…
-J? :½¬h®? g
°‰¢?ãÑZ¯k?̈7Xör??Ñ–(ã2!?ÊñËÇýí?Á¡ŽF2Þ?³ž®¯
é?à€àŸ‰0?³)Àu÷¬?ÏP;'23z?°Ic{3_?ίXûO§Ä?«€p̺þò?åDkû\ÖÑ?³Óú´9±?ÄXš‰EÈÍ?­~kDBµ?ƕµ‰FÛî?©}°¤y3r4FGL J1013.4-4006¿í¦,µÊ<@*ÆÜ~ñw§À:z6ó²äÀ<VL¹6£@]U¼ú@â@ÐO8?Õ7¹«?Á§ßÐ?ýxZŸˆÆã@Aï"¿ïðõkQ‡²?ïmÅÖ8†Y¿å[¿¤Q¿Ûìü=3g¿ä\°ºv¿ïÿø¨ó©°AGNbll3FGL J1013.4-4008NVSS J101319-400549?ïjbïcQu?ªÀbIŽð?eúïà@÷?‡ôÿ"µ?èë3'Ã?¤ñD2­àñ?ï?ZrÓ8?Ÿ`ªÊü/?ee¬ôb?t™''ž¼Î?›‹_#–¯?K'7	?íGI§ÿù<?™¢Ñ£Š}F?"%ð½•Y'?p÷˜E~¥?³@ô¨MŠî?—n\¦apo?í[dÑo½ä?'ª?DÎ?"ý×sóCŸ?|_;*ñÊ?°%c—…?þ?CæÉ°¨4FGL J1013.7+3444¿Ì-oD0††@KÉë têŽÀ:2Ÿ|àÀ<o©æ÷n@,­c%`@!þÍ?¹?½CW¾ä?ÀoU®2X@YO?Ù@R5£zîß¿Ó3ўm¾Ê¿æwÏz&6Ë¿åÙ¾bPØ
¿êÀÄyA4¿ï÷?œÎ€?Âø<èÎdAGNfsrq3FGL J1013.5+3440OL 318?ïÅDÆsô¿?vå  Þæ?[ìÒUyþ?[Ö'0,>Ã?vbhBðBQ?rîô™¨µ?ï2)cÐe{?–*4hÁr	?bOü&/9…?tîYE°è,?—pÔ-ie?"|¹áš?îùã;ž.ê?…×—¡Ô?r¨\»Ãî?`·ˆ€™R
?œ]u±½?ƒö£Z@?ïpù¦ê¯?wÙRžL¥?|'?r•Õ?ix۝ËQ<?…¾Í<L	S?qA4÷[ØÙ4FGL J1014.3+4112¿ïÕ¼Ì	êv@K{š¿4À:'7褙¨À<"þ)f+@{"Œ¿k@	ÒaaCè?¸ºt_Mm¿²æ I»O?ön"¸‰Hé@$Ž³°F¿æZùý‡€¿ãŒ¢~š¿æÈZý|˜¿á7ÏÆl`¿ä"'É›À¿ïú®‡ggîAGNbcu3FGL J1014.2+4115GB6 J1014+4112?ïéD†Í?wÑ>)´?Kh?vLš3?B7?'Çac?_ö'Ìl?vÖ32w?ïŒÐ6f'?ŠP·ãõºg?FüMã»å?TO¡ x½?‹cò¡›z­?ˆø|óK
?ï=­6·_Å?z_΂cwt?fŒ/Àµ5"?QŽ~ù/¿é?•xÓ0ý`"?x"݉aA?àǸ?r}+œ{?n©Ê'?`'îœNE¡?ƒUЕGŽe?lô¯¥ µ4FGL J1014.7+3210?ïñd³Ö(8@Kâ­>'À;[HŽå
±À<ÓESÇ'q@ x|l75Ì?ö»Ò©…Ÿè?ÙV»"«P¦?ØmAKúªV@cS;ç6Û@¤tz{FG¿è…¶Æ'¿éÛÐ`U*T¿Ü€("X"¿¿¯'ÿ'¿âVbýüÁ¿ç½®(`qAGNbcuNVSS J101445+320725?ï¨Òkßk?…†%þRW²?H–üp|œ?Al/Ç¡?O?"B^di?…5gúÌÄ?ïd.NœŒØ?'¡` ?ì?Hèþ¿_Ò?Yq­ÜçX?'²î6sl…?'.`M?í²ôöÂ)ö?—+Ÿæ%ƒ°?'¸'Ù%Â?uۊTjqÁ?°U—³‹'?•›êYÆ?ï
ÛJ`Âp?"fg\b
?P捞v•?Lh¥%þ?–5‹
ʀ?ƒÚ2=ÝK4FGL J1014.8+2257¿îA˸m÷@K7=áâއÀ9þ†åÀ<XnoId@=!¤W
@Ũ¹?º,Ö¢¹}æ?³yHÁ9ñ"?ò…×Û(@ûRK§HY¿ÊœdzÓÜ¿åfâÂØWE¿é¬u>p~¿ïφ»p"?àË1¡ã•¿ðAGNfsrq2FGL J1014.1+2306OL 220?ï譈(B!?e²k'à?X{"1¸š?Yù+¤°×â?V"tJ"?W|&¶nfQ?îÓí~+Â?¨Ò~™mïs?w_®Üý€?"º²Íçr­?Ÿ¼x@£H9?¡æJ:%®?ì0;—ù? D‰@ ‡Û?Ÿ1U¢£?z ¾¤?¶±Íא  ?˜²!™ã¼c?ï€6Ø×x,?dàOŠ	¡?hSê^S@.?l(¤ SO?‰ÝO2$â?ÞY›Ö84FGL J1014.8-0537¿î'ìxRà@Cúãq*À;û
͹\À<'@eJÝt@¸'r0@=ø{§@K?˹€ôM?¹Ç‡þç|&?íî/ªèv@hÚPCs?íÑóbb˧¿Ù3œÆtÄ¿è@ ìߑ˿Üñ±Þ‰ã™¿ë;<¡Æä«¿ðAGNbcuAT20G J101446-054049?ï2wd·ó?Œ›C÷¨¾È?b¦21×?W'Ñ]y¼?—{\M"Æ«?‹^5»´ò?ï¾k*Ðü?"klGRì?_ØFVwF?fÇä16ë?šª®5>l?'ÅP¼²Z8?íøÛIÝjj?"'‡¦Ü®?'P¤Œüó?uo°$jíå?«Þ"?!Ú,?´{ý?핽«SI•?ÝÒÇÚ¿?ŠÄm²;N?r)'êì?°ú¯kó?Ý|•ù4FGL J1014.9-4508?îƒÓ'Ai@"Ùº=À:VR,†À<5'Í»à@	#Îç.M@bE¿ý±q?¹‰M-ZV?¬½™P?ò_äÓSÐ@)Ó)]F'?×ÅUŸ™¸Î?ëàÜ^e;¿äV$ßÞL|¿è°d‰Ø[¿Ö}ÓLKˆ¿ä¼†~3â†AGNbcu3FGL J1015.2-4512PMN J1014-4508?çlò®?À\§XwÇ?—
'öëñ_?'8+h¸?Ðm"¨ƒ[?À.lðТ?ì¸yÌY?½£†à£ì?j4¬ÍÊ,Ë?€Œ´êÑèp?¹jŒ9i«Ü?½))¼Ì•–?èÊͲar?¥è?N†ˆ?Ÿ2{8à!?ˆ?è´ÓT‡?ÈîyÏw–3?£ÀÝzà?îjã4)4?ŒÉb -?]«AžªÏ?'jµ>IfÑ?¡"÷i ?"I Ôø4FGL J1015.0+4926¿âN
Bøg@J[9&A³À7!ÄÐoÀ:ùxiž)K@¸>Öªq-?ûþ/Egé?ŠžÔí?¥ç¨ß÷eÁ@WØåó@Yy&1—þ¿¶!x˘Å3¿ÔñëÀ-@¿ÛOqtõ¿Ú"fÝ.ĺ¿àޕÜär¿ØñnØ$ï¤AGNbll3FGL J1015.0+49251H 1013+498?ï÷Ç7D?†Ä¢ÿý½k?7¶]?y*?4(Çñm?‹ÄYÄH3'?†œ»p?æU?š´‹˜‡"?a¸ö''ÛF?p@Þ¼j¿Ñ?š&®²Ùô?™ug·Ñ×?î^͟ò©g?›‰.é"çê?€ahFû?€ÑeG¨:?¥úËïO¢À?™%>ñÓë?ïÚlP°?€Ä¼¯G5"?K´s~¢Ú?BNò\?ŠÎ³éÐw?€²jؽ4FGL J1015.6+5553?㓪ú•@HûìÃã?À:`"ՔÀ<®¬&dØ@vÀ7=.	@Óû¶Å$?¼3Øt »Í?¾šNʓb?þÞüz9'@ñµh'?ïõd›‹a¿ÕUšü›¥¿è2ø6#¿åEŸ¶´2¿ïÿv½Ì~É¿Î$¡Š~ɊAGNfsrq3FGL J1016.1+5555TXS 1012+560?ïË$÷˜c?ZDÅAHm?f£G]¯=?r-›¡ÑNþ?n7Á
Sì…?‹%ioð?ïks¿Ï?":)¢Á&?\cà´ì0?r"È×x@?ËV¯Ð×4?5ˆ^Íþ.?+»¬U?žpH¹Ê?ƒÂðô²É?{QÛ~^…´?¡W¬ˆ?ŠbîpPä?ï¥ÆâfÔ?pe‰'Ï?{bÉ'ïc?i`
)]‰?q¹ÅÐÝ	r?_Âέ‹æ4FGL J1016.0+0512¿ã¸™5_w#@Gƒ*ZFsÀ9Ó¬ºÞŽÀ;ô{/PP@/Ô®Bž
@¿û}º@?§Å#yñw?Œ¥'ÛÃ?ãŠ
jKÎ5@ÇÑb³©e?ï k°RBÿãxQ [ª¡¿æpÒÐòÌ;¿ày7Ó¬¿âAØ}7¿ê'õ¦	êeAGNfsrq3FGL J1016.0+0513TXS 1013+054?ïâ­6yï?gÏA	»J²?1P©ÐlW˜?(Ã<|ƒù.?k¹=x"§?fñõv'Ʊ?ï°ü*ê4?‡¯N¯òá<?9áÕøkt`?Kðò¢È?'ññ'%?†ÜÉ¿´.u?ïYŠÈ.û?ƒñþ(;Þð?m)=@ÈÚÈ?[>ӝ?šO¦þá=?'F쐍út?ï÷˜á9È?B¿"Ú
ô?iF&€õÍ?Þ¼…¢‰?P9Û$_s?BEU·¼¡4FGL J1016.4+7703?ނºytF@BmÏÝ"…fÀ<€Ä"(ï
À=§s³VB@!À˜ÐÆ×j?øêܝ$h•?áŸ!"OX?ï2€áü}@	å¨ÃÙD@ÐEìO¿ïÿ.ÿqå¡¿×2ê£whí?ïÔ*pìÒ¿¯ÓÏAé{Ñ¿ÙÕõ?‡ªY¿ïÿùŸé"ÚAGNbcu1RXS J101647.6+770239?î&ù:âF?»J¤ïF‰;?ŽÃ(·~`?†ñ-gÀ?¥ß¢0Ò;Þ?¹ÁXîߤ›?ìbBOȓè?¹ÿÃÚ?¢ƒ~}iu?¬òß0ò?³¬.C¦9?°*(ݨûï?ê¿¥:ŽUg?¨xžéëÇ?«êÑvi?œkåÀwòæ?¼|`ÂÒR–?¢pԞ¨ª?ì¸vˆ2¿?ª¤;ÌÑËþ? `…Cå}?˜
KŠ^ä?²	ww'?¦²Hy'`¦4FGL J1016.5-2650?ÕY†^m7@8oawêiÀ;2üÁ‡À<¥D@¡°¿@ ýçP[¸
?ÿ'6¾ØîC?Ôï˜ß_vˆ?ζ`dCÌ^?õr-å˜î?ý:¥¸‹Í(?î'ØÚø¿ïøžwNëö?ïÿ¡Ö~ý6¿Å¾´Ü?,¿ìè=Öû#ø?»¯d9ÕåAGNbcu3FGL J1016.9-2653NVSS J101634-265057?íP°×Òø?°+T6c!¢?….IY¾¨?}
ýœ°Õ?´§ºp0k?®ÚĖj/?í¼åêD®^?°fþ9+ŸI?‰Ž±'Hɪ?œTA3­VÇ?­ÍõâçÄ?©œúƒ²=?뫛‹'þ?¡p9÷»x5?·+1ç¯?^úkø\?»5XÛLà?œæ"èXµ'?ék¾º$Ýó?±/C8k?˜pºhðm?"¬£¦Köô?ÇBíÊNz"?°iՒ¾£4FGL J1017.3+5204¿ÛÏj湚@Iü¦\ö{À;†ì"øø¥À=š‹1!
@ ¦ß¢ú@?úpŽX÷ˆ?ÓCâb¶-¤?ÔÄO»)6Z?ûj÷	·8ç?ù&¹Ã_¿ßW7õ9Ó?á£&`;ÿà¿°Xߕ&mR¿Öƒb¯É¿à¨Ž"'Ùd¿éҜŸÞW9AGNbcu7C 1013+5217?íüín¼½?¡Éñr«?~È"†Z¢"?uµV3Áô¯?¬X+XHßÛ? ýýÄ?z?îËûaÒå?£®ö¸PŸÔ?­3´Û?…¡Ó7t?ªóý$e?¡!Ceù]?ìeîx¶^M?¡5U™¶ÉÒ?"PÅxÒá?"I¦õ\Z?·ÐxîØØ?ž\Šmp?ëÌZ×¥7/?™xìt4Ö?ŸÛ›|"?‰"ç384?¹¦B'Ò§c?–&Áõò˗4FGL J1017.4+2538?äÙ÷5^º(@KÏ\WìÀ;Î²€À<ʴĘJå@#mükJü©?ñxá'ͤc?Ù~íEé]?Úu$²?@Áù£Åm@¬3ÁM'°?ï»U
ôOÉ¿ïæòåˆ[¿ïÿè«î0?ïÿülò¿ßÙ%ÀÙÏj?Þ"ø!å-AGNbcuNVSS J101724+253955?î‡_㴗¤?¦!ºxyˆY?pY58ã¥ð?n¤"Vña>?¥~Ûš?¥¬N½¨?îÅñéÒЧ?©wpGØ??rûµFe-?"ß>RáŽ?¡AjºRÿ?§oI¾o?ì_BÏŦ®?¢H¯Q[ãf?…ÞoӔ€?viC%ý²?ºb³ØWû?¡ªB9Cz?ëªJ!®az?²˜áLmû?….AÊf5?•ÃÈáŽ1?Àó\ Å?±¾ŽU•ÏÕ4FGL J1017.8+0715¿Ôïm#¹™@HGÐ|"µÝÀ:´ÿK¥À<N°ªWVÿ@·ê)))@ÎɟâÚ?ÉIO>ׁ1?¹þ_ýý­|?ì>m=ðüW@
QÃu‹~?ïûŒž"#¿ç?*¸:o¿èÒ¤Uµ>¿èiʞõ#¿ïô£
[£•¿ãú'®š²žAGNbcuGB6 J1018+0715?ïî˜f}P?]Ö#"¯ƒZ?CÈ4ÿÎñ?G·*ûL&ù?XëÆìx‡?W±¤Cò?îüXý¶]?¡C‹jšøg?c¥
N?qژÃÉ{F?ž	Q?Fr—?ŸLiø±?î§ÒÑ×ù?ˆCÉpéW?tÅvB±:?eúý(¡_x?¢ê(:'ŠS?†¹cÏ&™?îՕ	W&?'1—õqÙá?'€-w·A?iÊÞٌ÷ì?œ
W?°?€ˆˆ0N<Ï4FGL J1018.1+1905¿ç"G¸{\@KÉÙÓEÀ:xàU¬ÛÀ<"eByø@FOo©Ü@˜0LÎæ?¹F½S³{¿ d¬Á®Ox?æîÆؤ@	rmœ™ì¿Ù·
bZé¿åçZíŒ_õ¿áá›@bƟ¿åP—&ø'M¿Ëªø;»lþ¿áTHÏAGNbll3FGL J1018.1+1904NVSS J101808+190614?ï–õêXG}?ZòÖÍs¼?QuÃÜ&ft?E^ëÁúƒ?ˆÌîiSØ?€‰PïqÓ?ï °|OÍ?†		ÚùÍ3?=êµ{J˜q?T_+º+ÏÙ?†ä‹@axJ?…œZ}Õµ?ï8¬à\h?ªš3åŽl?e‹…0ô˜?S"Ä¡j(R?yÁ.T??€¸–®gƒ?ïh3ŽÎžÌ?w	
Àü"±?SGN"®º?G5îSk?'À¹±CÛÆ?wЊºÄ4FGL J1018.3-3124¿ÅN?ö]@5ÕW2À9´¸ÙÐÁÀ;òŒVºø@zõ }ùÖ@°1;nÉ?ª
¹|
¿?®ƒ
¶è4@	Wɱ@iDû‡ H¿ºNnxƿᦕ€…K"¿è¸Ëž#—	¿ç×"'$€¿ì3bƒþ¿ïÿò(¦è7AGNfsrq3FGL J1018.4-3119PKS 1016-311?ï‰Æ…$À"?"p¤±û!?"t¿|ùè?>ïŒÖíd?r3>s­°?nÕÿ' …?ÉÊ?‰jÃN¢ïÅ?Yšµ',?i)h=È¢?Š¼Lº%Î×?‡3º€ró?îÜ"Ï·«?T"ø"l?…ƒ.:Y"á?~¥» q˜[?™»öhÜ@y?ˆ)õßÐÈ]?ï¦ýÏyP?m¬¥‹Ø§x?m~2üû?Ziæ¢Ã`¢?}ÂZ"ÅW9?fMzÞä4FGL J1018.4+3540?ïýebÁ|@L=
à"S.À9ÌQþ'BÀ<i­1üÒN@ðÇP6#S@G³zì/i?µÕRWeÂ}?»8­ªÑ$?ÿ»ê&z@±~Rû¿ËžM]€ä—¿áݑ`eŒ¿è« —ºœI¿æ@>-b9¿ïWàyQû¿ï•ÂH"AGNfsrq3FGL J1018.3+3542B2 1015+35B?ïî­ÃŸ?Xi.L*s?EÎTž‡~æ?C䮥'ú?W½Nrˆ"ª?SÒrÿï?¯²c?<yÆÍÙ?RoÊæˆ\?iÔÚEÚI?ŠÈfÓö–p?Šd€Eö™Æ?ï#ˆ\ÜûÍ?'7 –Èæ¬?vç"Dýî¥?tK	Rê^?•Õ+Ó!
õ?|ôÆÿT%u?ïâï©ÞÑ?WؑI›êÆ?]ÙÛKC?P/Ã÷B6¾?\H#'÷=T?KaÛü†~N4FGL J1018.4+0528¿ÜÈÙo"Úº@GÕËeè'À:,ßØBKÕÀ<öó4@O-\¯ƒ@uð¥)?ÂN…7x'?¸¨*ÕÁ"?öš۸ù@†ü®'ÎI¿î¡¢7_é?ïö€Z-s¿ä
Ÿ¥Í/¿åÓsD›:"¿áŒ	XnV¿ï¬¿EûŒÔAGNfsrq3FGL J1018.5+0530TXS 1015+057?ïÃJ©r/g?r¥##}»?TðÞÞ¸Ê?L@hMH¥?ys:F8?qѪé!t?úV$ÿ?ˆ977É°T?J%Á×<Ö?UwGŎ]?Œ3¯~YLw?†Ü-(ŸQú?îf]Bcá?'J%™
*Ñ?~3£Ú
?r®_M!?¥Öã·^qÊ?'ùž%²¿?Á'À?…·®Ž0Ó?}¥äbâI?lú]£¾°S? ÂWfG£«?";¹º—\\4FGL J1018.8+5913?éM:ì@HIÚßµÝÀ:›&Š®DÀ<Ì_‹€Ò"@¥¿â®‹?ÿ•a%´Å?ÀòBÒãg?¾o/êÖ?ÿk/=Û,â@{Ùs¤<‹¿Êk¯¦vKâ?ì	ÒÄ]"¿âvIh(ÞF¿à©RtA}¿ßˆn ¿ïÿþBe«+AGNbll3FGL J1018.8+5913TXS 1015+594?ï͚9I}¿?'qE1%ø?j¼æÖã|?w	'í^l?g©¾Ï«]1?o¸rLÂ[[?ïFFºj"}?"Í|‡4
†?c•¹	0?pâÝÎ¡'?"Äq'«¯?'
PñV}?îZ†¤‡³Ì?‹3'£³ˆ,?~'z<q/.?q=¶x+á?¦'¦oöP?‡'¨÷€z(?î±`Œô¯?ˆ(l'?–·}]ßM ?'\ëÅ*?"$֐'û?zJv'֝á4FGL J1018.9+1043¿è?Vx÷Qu@IMæ`ɊÀ:ÆIéXÎÀ<f,§þ·+@Éáš9R@·S´Eí?ÑĬ{*C?½è""¨¿?én
ŸOæó@—©Tw¦¿äÔ§Awï{¿èôúþ¹Xý¿èú³$…‡¿ìÛÄanYû¿ð?ïÿ—ŸïI$AGNbcuSDSS J101857.97+103625.6?ïÔ¬}òzí?u|K¶ãÎ?aÜVXó€)?eÛíÏÎ֕?iw+´''¡?l‹4ÞPz?îlÙ$ÖR?²ÛÈàŽÊ?zç;Ou\?‹ßb$ð[?¬|KÃé@?°sŒÇ~x?íc_OÏ?"ÀK)Ø?‰åƒJ)?yVPW* ?±¨WTAރ?'Ë!3"š?ïp|NØú{?€tyUó[?dSX*_Û?WnÚ_?ŽÌ?>‰+?~\zœø×P4FGL J1019.7+6321¿Õ®çé!°ï@G % …²À:h!È`À<'ž1Ún@‡-nÎõ?ÿ
ýÌ=[?¼]Ú{·?ÉgÒa·*#@؎6F@"‹½¸Þ?îísk1§B¿Í¶†9j"Ù¿ÞMdºã¿áŸ°9F¿æ˜f^ꖿðAGNbll3FGL J1020.0+6323GB6 J1019+6319?ï &xór?§ŒÚÞ¡?všª1©Q?>«<ÙvR?yRT@´? g56€A?ïN|¶ÂŒE?'Á`}Ù?Zîøbý?hÿg+Š??"y¡Œçv?BwΠ)C?î,á[$Ý?˜…ºAù?™!ÆÁ—4Š?'o§ï@? ¡é'Ö?†¢"%`'k?=è}?'eðÿÏØ0?ˆ…†Zêâ?rH]Yš¨Ÿ?œéÕzîò?|BT±è%h4FGL J1019.7+0511?Ã0Рt‡Å@Gâك"t—À:áüjIJÀ<pšäó4@@ Œ£jRÚ?þú¢
¢?ËÌÆÐ&?¶IÏAq9~?íM	""}Ì@
!N§-¿Ø©Ý´{/¿æÀaïß Œ?¡x­™W¿ÖÞ¾fØ|-¿Ú<XüŸ£¿ê<þޗÐlAGNbcuNVSS J101948+051327?ï†SF%
–?…ó£Z·?9÷•Ÿ"Æ?:^Há?£º^4?…x"#]Um?ï™î"OM–?"zn½uê?<ÄÓçDù]?MÇX)ƒíê?ˆž4Lòr›?ƒ»¡DŽ@??î=Ïõy*?•l¹sð"Ú?d¢ÿ`¯?[L@O'w?ªØÞîF—T?•È?ï&°JŸ]?}{ôR–?K눞0¯>?=8£­¬r?šJšg"Öð?|À­épï44FGL J1020.7-3920¿î&V—w'˜@-¥ê«%)À:õgXÔ­lÀ<"UàÝ%
@ dæÃC?þ*™Eå½?Ê÷ JÂÌ?½Ù!™Ø®­?ôä$7í'@ÜÛNšÂ¹¿ïÜ>Å7­?ïâÉ¾²¿àِ"Š¼¿ÍOÿ‡4<H¿æEz=]Ùz¿ä¥ ¸ò¥AGNbcu2MASS J10203893-3920563?ï5­õyË?ž[T4Ҁ±?_
ÐYm·?•Ø.æœÆm?—Y"VyíÓ?–+Ó}eŠ¦?ï0£›ÿ¿¿?•QéI[™y?\¨£mÍ?iš
l5â]?˜+aõÖa?"T@~ûÚ?íÝBª€i?"iÞ$êÙ?x?H/"I?dÍ 5Eƒ;?¯''Ïs¹X?':Lü«Ã?íÊ*ï¡?'-úùÆÛ?‹jûm²^?u'Qԗx?°–O:̨?Ïäº]V‹4FGL J1021.1+1626¿ã€Ñ9v¡Ð@JÕQa£ÊÀ;cüÈ=À<ÇG&/>²@ Ô±šA_F?ýàA8¯sö?Ó? ^¯¸À?¥Ïƒºþ?Ëáºö¶€@nÊ£|ÇQ¿ïÿÇ*Ì\e?ïÿ<‹¡‰R¿æ‡9zu$¿Ã¢ÓÔþÊv¿å­å˜îy¿Õ¯=oÍAGNbllSDSS J102100.35+162554.0?ïØì±ÍÂ?nSÐ'­?4+g«u†?0‰¾½'\ª?rFðžfã ?m1+ò›Ú1?ï'òé?³?";\@íHF?Fi‹Q6}?S—­АL?Ü¬þž_?'Û—e°Ôž?î2Š•%?Ìh¥l@`?rNç'éß\?]Újal.q?ª"Jdr±×?Œ¨{?îÔ"(¿Ñ&?…ù×ѵºN?qu-.³Õô?bi!1ŒN? 7Î,rÝ?…óG×á54FGL J1021.4+8021¿Ôi»ý¾ÿ|@AM˜ˆøbÀ:W‡¦RÀ<˜ƒÛÂ3@"¸_˜@vWu1ÛD?»î›~¡Â?ÅӊV/·@~ɄBð@?üo5JÁå¿Ú¶ÇÝyÃ:¿ßWsÄÈÇZ¿ãd.]‹vk¿ãºPþöſ×øz?Ϟîm0…AGNbcu3FGL J1021.8+8023NVSS J102201+802350?åتÿa-?Á¾µ?m"I?¹Q€z.?°RáR;ú=?Ì«B>›:?¾Ï'5Ý	
?åvwö"?Éä%e稈?ÇEFG–G?Æwҏ7Ռ?ÂàÚà™¤?µ½H†D³¢?闣 z;V?¨r·³Û²d?³ð¯A¨5?žÍ¾÷(6ä?¿R3º…ð.? àÕðßï?èÕNÞd)À?®x6‡Çþ?ôóE?©¶S®´ÞU?´¡ø&ì?™	í7êò4FGL J1021.9+5123?¨O\šÆÑq@Jt×I''?À;҃9LÀ=Š'¥aN@ƒ{³žÇ?õ¢Œ¢:R?擥cÒ7p?ä³øà¦ôK@¸d"@úø´‡0¶?徚À
F«¿âs1fªY¿ÞçÂòXx¿Î û;;¿êFJ'Û¿ïâ~
ÇÚAGNbllMS 1019.0+5139?í=~OaU?­ÁT¼ð(¿? µzž´_˜?E•ùté?«r£ìU‹.?§tn׶‡?퓵s)?±®Ê¤/‹ô?Š_Åna¾O?˜¡Mí>v?°^‰P.í?¬fyÇY?ë%Ý&yü?£àÇ¥ØøO?¥8òÙËì¹?'Œ»åÈ4×?¼:Ï©æ9Æ? ?µd]?ìøz¶Ðm?¡ÄÊyÆz?~Î*†Êµd?ƒ¿"nzg?¶OG¡ì4?¡#ÐH(ôb4FGL J1022.4-4231?è 06©ŠR@(¶Žæ¸0^À:\a5¤ý{À<^~ø-£§@4Ö ˆŒ@ª"£hO?ÀºIýÏùþ?µÏ?Š?öFB‰èK®?þ¤ŸÔò
I¿ÜÅÄDèè6¿Øä2"Œ—(¿äU.enâ¿á=u×H¿â°T[¡çF¿çYº¼)›AGNbll3FGL J1022.3-4234PMN J1022-4232?íYlEáH?¨·úK-žn?yáaŽWtP?iƒ!eêçô?³–‰,ë~|?¨@@4œ^?í]~Š!mï?³jåfkC¿?x|Íb¾)?ԖZlä?³'³âd¢?²ƒp¥ŸT?쪡÷w.?¬ K±Š?‹f%o9K?vëpKÏ)?·>+™=ë?šî#A°/"?ìÈ\bà?'SNZ¨d*?–g{ü]úV?|á‰5ÛŸ?´#@
Øzv?ß°¢2!4FGL J1022.7-0112?ïhžH™»—@F08⟜éÀ9˜püÀ<Sq@€bÐãå?þY·+zØ?²ã2½—{?¥(+Ã'\?ó{–^{¶Z@ôœ"µâ{¿äÓF=üåÄ¿á¹\þØ<¿Þ2½—z°¿Úv7_ÞO¿à‹aÝ냿ßä€]2‹AGNbll3FGL J1022.8-0113RX J1022.7-0112?ﷀÿÏ{?s–iÚ þ}?RiÒÞlÍ?GÈÞ̪º ?¥`» ?qýÅ
0±?ïj 
|c?Ž±+Å8'?V˜î¹9q(?c]×Rù;ã?'Sm¼Ü?Œ5È¿+?í®&ìMþû?"íw9]?'ï¢`¬?qúêºâ]?°0å|›¼?":Rוm?î$¸Û¨‰(?Œ:ˆ,žeF?†‡<:>8?pœ(‰þ?¨£6óË?‰WÀQg4FGL J1023.1+3949?Æÿ&ˆ¢Gà@Lo1½èÀ8ßÉ#ÊàdÀ<"àæ_E
@ŒÊ(W¸@ùÅS[È?¤L/¿œsÐ?»'Æ€FP5@ä­Ýô<}@ü9§¿Ì†ùXñÞª¿áíÁ9ÓÁ¿ä'ÙaÏ©¿éDåw¾}¿æV†''>¿ïÿúŒ—ÓAGNfsrq3FGL J1023.1+39524C +40.25?ïÓ§yÑâ¨?‡†»Üë§?J¶×¦æ5?H5J˜²åÉ?rÕh"1Ûµ?‡Pû'["?ï"ÊÊ	?"–ÕÌîç?J¿"Õ	Ô?^Ä>Á2÷?‰!gÀ--ý?"#…ï›s?îàjå}×X?"Ó,C@Ÿ?̔qÃÌM?'¬ø<?›ÿ~3Ô!ú?'Vâê-'ò?ïýyé;z?'1Ènáê"?t­À¢2?=±:Šk×?1›Ìð?%¾ÑM;=4FGL J1023.2+2859?ï9U¯	@L²82vtÑÀ:ªÐ»nÖwÀ<Œdý±@xšô¬·@uX'?ÏÕ£5#Î;?Ï?/*ee?þˆýՃU@™½Uá]þ¿Ú0œ_ǐοÝ&‹º³Å•¿åâ,m®"¿í½mHضæ¿ÚØïþ¯¿ðAGNfsrqTXS 1020+292?ïpT0é?"Wc^ê«?mÍH(Ջ€?sßrƒå{?ŒiXé9$?'ƒ.›Ðz?ïþ—‰ª?–÷0O³Õ?c-nŸ‹5Ã?oF̋ ÷Á?šZ:ÙUå?"'5d—c³?ìôÀΰì?šm"-B™s?˜»;j?Š®¼ç Ú·?²+0†êµÚ?'üo‡‰ì?ï[š{R'?z¤ÖÅ­›þ?r&áÆJ$?e°¸Ë7ÅÕ?ô?s?vÕÙ©mÏ4FGL J1023.8+3002¿â\8Ì5‰@LÍ®>lLYÀ;)€z䢬À<µb+nBÔ@!7¡¬ãx?ý´òd/U?Ç}ÖZHŒ?n­àMˆ?·¸Ñî×@€Qû,Ý?ëÔD$òþ¿ç³VÚh¶¿æg¾U:Å¿ÒÙ~ —O<¿Ô¢ÃäÆ¿¿à§".ÍüAGNbll3FGL J1023.7+3000RX J1023.6+3001?ï/ÝÌÊW?¥y5Y–®?F4ÑÍ?PRp1V¯s?™OÆ=&Æ?¤žÞtK¹ë?ïmÿt¸Ô?•ŸçWq5T?Dm§m$?Q´A®¦#?'œ¤Cûü]?•\±Ó¬?îKöäÕé?'£à?fø~ÿ<8?Rù…¬µ?­K¸¡¾Ýó?'‰''Ãm?î®'ù]`1?‰j÷rfõ?`&V¾ƒjR?R)Ù<Êm ?¤þAÆ]?‰ë¹Ö_³F4FGL J1023.8-4335?ï¾nš^ÝÓ@'3ó.ZÀ9"Üõ)À;¸•Ew–@ 
½Ál‡?ù¬gíO#T?°9?硏\?¼ßyLȼ@ º}>ð@¥['¡'­?ï÷=Bÿ¿‹â꬗ß@¿Í/?ɸ3¿×•)<ºEŒ¿×úžAI!¿ÜÞ&¼W^·AGNbll3FGL J1023.9-4335RX J1023.9-4336?ïÂAÏ4¹à?|{D7(?N¿K
7I?L6˜Ö ÅÑ?{/ˆØ?{ðXH!?îŽ]´b]È?¬÷–Ä4^?a{ÔÅåRÓ?lCõ+a?¦gm{ÎS?¬r'™ï&U?î8£¦nƒ€?—7m{¥­?…ò­Ç¡à?…èÖ¿k~?¦ùBm¥ßk?'mWå¡?ìÃ(WÀ…?Ÿf¨âHŒl?Š"·ADØ?oÎM^œ6?·µl«®ž?ŸD‡^…4FGL J1023.9-3236?ï÷ø5A'@4½Þß)À9høH{™ÔÀ<h;R¼@ÕÈ<DSí@Yú—á2µ?°¡ŸL‹ôÀ?¼ODyׇ@ "Ú@¬Ûù Ý¿Óå•ñnlÅ¿âã}_*Þ¿ç‹1÷ÉЙ¿å¨âaßn¿è¤Pwؕ¿ïÿ܎᯳AGNfsrq3FGL J1024.1-3232PKS 1021-323?ïöü"œÑo?\øŸ³ãÊ)?4çÏ#ÉR¢?2NT`X£?Išú՗Ì?\|z‹Fñ"?ïÆ}ËÁ‰6?|ºtT>?@Θ–"ûö?S8ÇøÁJ–?z§Ghå(?zԃñR6?ï…ufÆ$?€õOzý?uh´ŠÞ 8?mI·™An?–µ$0o³"?|,ÍÁâÇ°?ïôÔ«"D«?A´åñ²~?(ÚþG?ý¯&–)º?ST­y³'ß?@[bξŸ4FGL J1024.8+2332¿î8Œ¨3T/@Lf/¾3¬ÖÀ:Jº))À<'ÜÜåHÅ@ex?V×þ@Ë\ŠD'?¹ÁHà®ø?z™™øÛ?¿¹:^J¹@0g…JW<¿žóÂbe¦¿çy€‰þ#¿â˜ ˆ5Ä¿çJ†¡oPñ¿è_ÊÀØøª¿ç_·¼]êAGNbll3FGL J1025.1+2333MG2 J102456+2332?îԁÿ®?œœºÊã?saëš9	B?hÞTªˆA³? K²½ýÐ?›÷uœ†Ó?ïbÔ,–õ¤?ÑÒ)WG?U«å¶±?còÁ½(7<?'Tï®Ð ?"÷Þ3?î4Fžx?"¢ýŠ‰ŸÚ?~"ø^~%?oBÊOÄUù?¨í3è¾?'­Tö?ï2ã}œ­4?mÇ+±?ìýœÁÌ'?i¸¾Kž?'¨På9æP?yY=éz84FGL J1026.9+0608?à±iR:F@HãBEõ­—À;éuyÿ À<…/PO¤@"êvÖËÿ?úG«<#?Ƨ0›~K5?™:"£§?Ó/á»vc?ýÄL`*ã¿éøÍ ¯¢ð¿ï—eýŠÚº?èËb¿gßb¿åÉ8Þmß?
^b`ó5¿Ï¸fGÐAGNbll3FGL J1027.0+0609NVSS J102703+060934?îWÚaô¿?¥\œ	ë?O´rãͳ"?CS¤ª÷—?ªŽ.Q}Q?¥<µªR#â?îÙC?¥™À·¶?cܘ'…Š*?s[«ñäí?¡.V†ö?¤"ÝÈ_ì?ísÄŸ2×?•˜æm°W€?v*ØL,ûØ?dâ*í9íè?²ÿ2C™ƒ?"žÖÑÔ-?ì|-ÎD&‹?¦›Ê¤ˆ
˜?`Aá™$Ê<?`ɞÑõÑ?»œ'¥U?¦¡y•<)E4FGL J1026.9-1749¿ï†Œå"@@',ºs-õÀ8ýN.KmÀ;ށOøÄ@¦'¥¸‹?þ™‹Ýtk?¨ý?l®?Ÿ-ڃě%?ôÈØ앿ð@œÜ$¾¡?ïÿ"­~ÿ¿âöq ~¥¢¿Üœïd|Vh¿ÜÂܾ²W׿ߣÂèG|–¿á[íœP-?AGNbll3FGL J1026.9-17501RXS J102658.5-174905?ïó#]‰åw?hý‹ØÈ7
?ªK•Í8?ø¼ö]¦?XN 2Ø=ÿ?hh7í$™?ïµ>ㅛþ?!¦ŽÁ
õ?A~xnp?TZ‹ŠÄ?˜e§ya?ê–}?ïIˆ,\|?'ê"5x¢S?jg4O\›E?V'ôЫ?™éèpˆÝ?ÇGÐ+î?ï¤F("Æ0?q)hˆÐ<?L2ÀH°]?9ßk¸YžÉ?…+IÚyèý?pƒeDÂt™4FGL J1027.0-8542?Ãóû'þ'À7£é·¿ŽÀ9VFíû¾À;äé@- .Q?û£®@˃?±«bï¹`ß?´×mÌ ª@PÕ¥¹b?ë@­3J¿ÕTF=Ñò¦¿à@GD¿ÛQ'Ã'ë¿ÔÁä×Ût¿à(»àì?¿ÜœŠâAGNbll3FGL J1026.4-8542PKS 1029-85?îÊ
6?™G©SEÍ?rs‡ðR2)?pE>R9ÅW?¡#öf?—+¾Âbõ?æ%Œ»eÀ?ÉfÄg¿õ?ÂðÇý8*?Ä÷Š…Ò#?Äz¹ÏÚgÑ?ºì
5û?ê?¹a]éM?¦è¤5dÂf?›æµey+r?Šnì'jª?ÄCÍÙ5^?¤}ܼÆ)?ÝJÎ~½g¸?µ}JºÌž?·êô8=??¢V 'kZ?ܺ­Ä4ˆø?·WMP#(x4FGL J1027.2+7427¿íUÖ.S9@Cšù jn3À9Pý^e%À<gŒSã@rªuÛy@;'}E¥ü?°F[®ýY?µFÏóî@g‰¿1×@.[~?ëÖz•ÈSÁ¿ÚOŒ…4î¿æ!pÞ9†´¿äñ"íjÒ¿è…?\ŒH¿ëKã-abAGNbcu3FGL J1026.5+7423GB6 J1027+7428?ïÊx~÷¹?s–·üsèf?S"ýÅl"?OªWU,db?uûžï?qtU"g?ï'×uh²?…ºÚ1ƒ¦¥?Gb¬"81Ü?ZI"´}Û¦?Š÷Ü»?"¯x¢%™?î»òI›;?‹¸tø…?|BB²UŠÎ?p×V¶[˜? ¸"šù?ˆ-Úª}?ï"G‡øJ7?sYOD,	?m.¦ê'µË?Z»	œ¶á?ƒâtGLļ?pää¸ô—Ÿ4FGL J1027.6+6317?؂C«j@T@G}"M:"À:;ðJ€VÒÀ<¢w$ú‹L@²' V!J?þS¢úkk‰?¸ø*We?ª®NÝ]¾¢?ðïga8)<@lïåU¯µ?ïû=ù_ÒÎ?–'¿§í'¶¿ä¹xýAߞ¿Ñ>sV¿áƀ,‹#¿ëùsôÄb›AGNbll3FGL J1027.7+6316RX J1027.4+6317?ï ́<È?yò]l.X?`¨óø‰?TGW;¢ÉP?ƒÞb¢ìϞ?wJžˆÆù?ï,ÑC÷xP?"ðªwâ,=?føŽ"þö?s%1ßñ'Ç?—†×O@V<?'44Æó%¶?íÍ¿Á$Ï8?'¨SîÇš?«Sr~²•?pmÄ"âd?®¹/_ä?§Bž`Q?í°Ô9oÑ?'MسÀ\?¢Åx©æÏô?ˆì¥%V!ã?¢-C¿(#?"	¾zÍFÛ4FGL J1027.6+1828?ïÿ6²LK'@Kñ«ó8qaÀ:zXËs0yÀ<u¡Å¸•@œ_.
Ú@ÕIe¤Ÿ‡?¹ÎAÒ¿ªê^ƒ"â?ð­
ê¤@є\Ãп×wCÃÏ"=¿é"iÐË¿èӓZ»7y¿Û¢ëý¿ˆì¿ããðj`Æê¿ðAGNbcu3FGL J1028.0+1829GB6 J1027+1831?ï݆Àÿ]?oJå]O{?YŽ]}…u?P¥œiŸH»?e²Aà6Ý?l­±EÁ`?ïc$ù3Ÿû?'™ï͒¥°?VG…¼ž?eŸ´i¯¡Ð?'6è‡Ð6œ?ŒÂ"?î,®#f?‹ª(ê¼?ƒ&³ROi?u8<íFÎÉ?¨tÔËd3?‡–/ä£õ?ï20䥷?'<â\J?ƒ9y Rö?sԆ·yÄë?®Œ_?xÛ}œtm4FGL J1027.6+8251¿äßäÆW'@@hó¡LìBÀ:Ž‡=vƒÀ<¾|ŽÆØ@^Ç»ëÓù@é']e5å?¼±]Z¤k¿ò»Úó<^?Ôå¢;~±6@-W&,¿ã{ŒhX®î¿àèh~ïtB¿äiæ÷mŠ¿æ<Ý5Мe¿áe¥«ö"p¿âÖ ž9%AGNbcu3FGL J1027.8+82532MASS J10284195+8253398?ï©ùÏ-?†¼i£ŒÎð?R«|¼ðœ?Tú,WÓ?ƒd'	œú»?"þ¹F6?ケɎ¢?};LâÜ¡?6]Ü1.?GpOŸÄh?½=wcl}?{Òâšul?ï œûŽ¼<?'ôàfD5W?hÎß›sî?\üùA~ "?˜Ò"­•
?~¯µúe?ïׇÈòê?\œ-ØgP?JK6ˆ‰Ò•?7ˆ´Ýžñ?q6UJuPÃ?[OK±4FGL J1027.9+0252¿ïýù¶ïì@HÏÃøÀ:nӕ=êFÀ<A†l–+P@³¡ÀY¡Ý@õ±…H©½?¿ÿ²RM)Ô¿µ
…†H?ò¡öKKX?øâ£8SÙq¿ãa|¢¿ëZ¶ÐE®¿ìÐHbz¥¿¶d±Z€¿êê~äa"¿ïïK|ÖtAGNfsrqTXS 1025+031?ïí¥|7?°ƒ*!aÙ?‰±¶ÿà
º?Œq/(cMO?'é'+`s–?°\Íqéq?íÅ«a¯‰`?´›pÂÅ|±?úâ€Á¬?¤ju5'®|?«¦'Eù‡?­cêÆÞ
\?ìUöª-Ć?žÎ^Y'Ãå?–Wã­P´?‰ð¹ªÓkö?·ºˆµ¦‡™?›èÊ%­§?íz
-ó2–?§r*Œd2?£0+øË]î?¡Ðր)A?¥/(x¡?›îtÿÕ½Ô4FGL J1028.3+3108¿áMu@MOп "`À; ³	­'ìÀ<Â=U™@óF3@@÷U^×%ì?ÁÁŒ|Ћ¿—».>׬$?ÖÄzÃÀ‰@	¢ohî€ý?ècÆ
•ê¸¿¯Ù1½šÞF¿ç,$K8ãv¿á*`üš¿çN£Îç?È8ôhG<*AGNbllTXS 1025+313?ï°¥Rä%T?€Ø&´SQ?QaûE?E¡ T0C?³
ºÔ«"?€!–Ä}±$?ïœêæQµô?…"úL?>\£h7	-?PFzßm•A?‡ÒaPPÊì?"ºç•ä?îß}çx¶p?‰Z¼û2ê?ou'u }
?c{|
ÓH? Èq"'-?‡+Cˆb?ï–ôùÝ
w?ož¹ºÊ^l?aʄ"\íð?M¹ê5ˆã?…Ð c¦&Î?m¦ëü¾m4FGL J1028.4-0234¿ï‹€á@FB[åÙäÀ:",Ý®œ`À<YZ;µ¸´@œ±a;.@}G{¿"ÿ?¼9ï:
?´«§Ž#ïž?õ	Ggž@
Õd]͐—?ãi§c†¸¿åvæF–"¿è2ŒÖ<¸¿çwlþ°õ¿ìð]ºpT¿ïñÈdˆ?ÕAGNfsrq3FGL J1028.5-0235PMN J1028-0237?ïÉQ°€Nj?sH\"‹÷?Z+ŒWŸª³?QªTµ0DÌ?tÌD©ðá$?qnðdx¼5?ïl	;êB?'ò6µ­z8?V¿¤²ó_Ú?j~wWß¹?'Þ7áµ?fº5X-Ÿ?ï(Æ¥Š‡?€Ú¡†¶W?q4b¯q΢?^}õ‹ la?–š¢â»€?~sb\oÈø?ïf·¸)ôŠ?tôÔB0?yÉü­KŠl?b²Éù·Œ¯?‰mžÝj?p@êõP¬4FGL J1030.2-8403¿æÛ¿â"	À6:îA'šÈÀ:Ë£jÓ³qÀ<t±i@ k篧"@Â9櫛$?ŝ´†YöÁ?³Îð"{rg?ñBºtÛt/@Š²öâË¿ïÏAò×?ïýw$#Ë·¿ç	Ü!Ôf¿ãØҔŒê¿Þl¤Ùh¼'¿ä.1,edAGNbcu2FGL J1032.9-8401PMN J1030-8402?]}~?¦'`¶?X·[|¤?Q˜¦$nå?›à–'ˆ†b?¥ÿeAnÒ?îáPwÐ?›=†î?c
Þus½À?iÆø¥P¡? ºQ¸QG ?š*'öír?íÝ\F©?'¬1BÁÏ?yJIÖ­£³?eÒyI¼e?¯6Ÿeàù?}ï¯â'?ì&y"«åÉ?œ«ÁCo?'ßþá'2)?ßN][´Û?ºT3¢W,?U*%êŒ4FGL J1030.4-3001?î‡w…ȁd@7¥/Ÿ¾wÀ:—F·G*À<Wé^ÓÊî@ú#d=;@ÿ\±Ö§?ljCu –
?À¸SÙpõ?õ'ÐɱZ@æ¼,k˜Õ?ïyێ0¯Ë¿è"^ß´[¿çÔ/—¿æÒ"!=¿ïÿ­_I;³?î47ûäAGNbcuPMN J1030-3004?ïå×½Œ?"Φœœ'
?¬±ξ¢?Oåõ@"?"˜Ûtžü?'qBT9Âô?í½CÂx²•?«1vÖTcf?‹>^‰¤-k?'%œœO1'?­\,6Ëk?¥yBž©««?í­‡¥û'?–I¼Zv'Ç?'xØ>ö̼?•Õåo ?²ì]³pE?'ß"–Åu1?íuWéÂ
o?–îü
ï€?˜+èåDJ
?…VïÞ|×6?¬"Œñ=3ù?'açäµ4FGL J1030.6-2028?ï(Èÿ@?s̪ï,À9䌎\À<.'"ø@ ]>6q?ûm±cºº|?ÀªQø›1Ê?º¸p^â¹s?þӊ¦·N@:㫶}¿å<O;§uû¿Ýg"s—§¿Ý–±Ý³$¿Ðkž3²4¿Õî¯á»v¿çø
¢gÉAGNbll3FGL J1030.4-2030NVSS J103040-203032?ïށ¦ðÍ?dX' R?>ÅV·Ñ?60úœ~s?m¥¯$}<Ê?bç}‰ëo$?ï§oƒ)­/?ƒLÛ^©x?E³,I#"?Sï,šh	 ?"Èìt`"g?ëÙÉWéµ?î'øg?Ê9?UÿBÐ̂?p{JáH?eâN+oR?¤Á{Ú9?}UñúÍ?î«à"të^?"""O×>Æ?kàöÌÑy?Y؆ðì`?£ƒîkä2£?ƒX1|ÀrK4FGL J1031.1+7442¿äzDÃ@C™b¶®}À9×â[ªJÂÀ<7 Àiçû@ÒÛ¯"¬@j¶ÂŸLa?°/x""]¿ž¶eà¸À?ð_1£æúu@;ö%`¸¿Ú«Ä"o
¿ãóVµ{¿äÁ߇Oj¿ä¹mtw¡¿å°‡‡H^>¿'fU8Z~@AGNbll3FGL J1031.0+7440S5 1027+74?ï±ÍÎëh?€ÜVBç
ü?LÔ
õb,?Cpu•'h¢?¿K•åC3?€)´°
?ï!"~¹?ˆßïå5ð?Ij¨üÎË,?Wø–oàÙ?‹ 𐲥?‡˜Ëe ô?îô¥mßÕ?‰:&lF?k:\íëM¿?f,±T/bë?ž¦_›¼?‡ShÓ!)?îDzÎÈ=)?‰z|T?væ"ƸÃÓ?c3õ»Ëˆ? ¨z¥?‰6Ã/†N4FGL J1031.3+5053¿Õßåø[µ¢@K:\|ؙÀ9$wSôsÛÀ;ñEgée@ 'äõ8?úÑW%€Ã	?¨â¢:ìª?¦ÝäIk.@Ûh‹Ú"6@{Û3íÃ=¿ëdµ÷ž1¯?±¡ÙY"0,¿Ú¬)Ür\¿ÓÂNĉ1¿ßYvɋ¿¾|^pÐAGNbll3FGL J1031.2+50531ES 1028+511?îü)]›	"?–þÿŸ±g'?_só}ÇÇ?ZÆ~Ši?žƒ•Vñ9?–ܓ¡ôw?ï
!«?–|Jêͳ•?gäoÛØ?rٟ=øa'?›aAàO›?"Èü'Ð?ìLËWÝ°?£d	lwÒ?!ã†?€Üúy?¹þuƒ€Ö?¡µ9³ÑF ?ìʘN¨à?š§û‡ä?"À$øGŒÓ?|É6'Ëq?´¿ÁÿxÕÎ?—Wg$€;4FGL J1031.6+6019¿à"ù)´@HïÝëÙÀ9qÊ0:ZoÀ;ßþiýʜ@}'î°@ח{²(?³ dd?¡A¸~ƒ‹?ìEHßlâ@/]K4²¿Ç,ý6¡þ¿åh9Úí!¿æ9ÐÁN‰¿çk%@@¿èT@ßn:¿ðAGNfsrq3FGL J1031.6+6021TXS 1028+605?ïö®¸$?Ok†.?4ÂKªØ?0/Èú²aŠ?Msd%š‰?IÁRö'?˜À,?ŠSÔt?E=½¼›?VJ?–¨ÐÈ?‡þÌ
ô4?ˆÚFIé?ïe\ÿ×N?$.ÓBÚ~?q¨ßn³±Ë?b˜ê`6*2?˜é"X)Í?~'†L:O?ï°º†¯ë?mq=%L­M?ZS>†é£|?H»zFsL?€†öƒBÐå?k©™*^0­4FGL J1031.8-2609¿è"€ˆ¯;@;ÚÂXՄÀ;bÍÞDÄUÀ<©EW"&@!"«s5Ø?ÿUdìã2?ÉRß äçv¿'õžþ'U?Ëò{Gžû@=Ü.""?ïÿå(
eC¿é#´ùàV¿å"…fîW¿ÞTÊ\°¿Ùö¢½.ʿ͘uWEMAGNbcuNVSS J103137-260715?îÎxb…b2?¡˜j[ËG?U2ù[¸?SfáD>.‡?¢p?ß5?¡;ŒÕ\?î{>éöC?¥g+4µ?kÖ''Æ?{åÜßú+?¦Ž½Y>+¼?£ÐŽN'€ö?íŽ/ûDÒi?–"²C?r'tÈô÷x?]àYý¢Il?²fXÙJ:?•Y_ÃȽ°?ë±Wð£yð?£?of¦È?tòBö"0–?m»BÅ?À"%½v¸?£Ê!]>¥i4FGL J1032.6+3737¿Þ/YÁ´¸%@M‹ÐÐgŒÀ9ÞHÈÆ­ÏÀ<O[ïêß@nf'†*@°ÔcšL?·٘b7¿}ËކÒz?DzvÊ·ž½@	Â*úÕsº¿ïðÝî]@M?ïû¾½?'¿ã.$5inY¿ß:;֚׿ã/×^ G¿ÚºTDzÙ:AGNbll3FGL J1032.7+3735B3 1029+378?ïæe/L?•F &r†?7'$ƒ_±?QêñÖ	]?fŒË
dÄ~?".ôŸ"É?ï™l…ejY?‰UôŸdΜ?J!àxÌ?[5Wƒú¶.?ˆÀ¦¤±ó?‡Á5{¯Ì"?ï1Þú]ub?|)?stÓ?eDz¯NÛ?QØÙ¼–gâ?—*^g?zYÆ©ˆ?ïx©'åÓñ?ut³LÌ?vh–TE?aЁ¨ë´O?†¡T>`áo?qÓ¸µ"AÐ4FGL J1032.7+6624¿ìÏí
è~@F¦ˆabñgÀ:³Ò†ëAÀ<áN‡Lü@Ýòd@;bŸ1‰?Á-蛊_•?¶á@w>{?ó{X|˜Ø@&©b"?èø±Eˆ¿än"½"u˜¿Ü§A¼c¿â¿Sg†¿ä?_¼S-¿è?¸¢HiÑAGNbll3FGL J1032.5+66232MASS J10323905+6623234?ï[åœ"p?ˆn™¯¾2?c#˜òã?ZÜrd*""?'9™]U›?†¶nq-*X?ïgóíÃ9
?Œ(Þb#Í?N½%`>P?[D'eð@á?'"^mÜ÷?ŠÁƃC–?î¶J–AÜI?‡óÇ®òìA?r3¶dõ?iåŒÝ5™??¢TòåœÎ?…£®Î[2$?ï!¯§‹?{ç;ÝÜT?,Àc×ß?c"ÆŒx?"šõNB?ybØp®ìC4FGL J1033.1+4115?ºª™= –Û@M0){úLbÀ9ÖÃƓÎÀ<T²¡¨[Ô@¼®Ç~.@¢Ÿ§Ñ?£Û1ƒIÛ?¤ÚT¼ÅÄ?û¹St[@Úº±AV?×6
G¿àĽÛB[¿çŠèáÖIM¿â±ªÂ‹Ö8¿ëÁ+Cz©¿ïùá½õ™uAGNfsrq3FGL J1033.2+4116S4 1030+41?ï¹`àÆ.Ø?·ï0L½­?SÀ¹5ž‡?Lg½ä›7?~_aO£¬A?€×!åjr`?ïZéÐÞH$?™Ón®µ?bZ™)­²?¦:§­?'`º'ÅÄ?"¢á´¿¾Ê?îøýÕ(!Õ?ˆ†
z- >?uOý¯'ù?l¹ X]Y?›ŒE÷äm?…Ïe\A·+?ïÛI=Zð?cfÛåOää?gÎ*&¿?_)½®W?[KI0ýäÑ?LNõXœ®Ã4FGL J1033.5-5035?à¿Z/:D
@×ÙõÀ9¦œë]±ŒÀ;êÅ®ËZ@ Ü:Óær?ù4m)Ï?»t#ùYs?ÉŒv›gÐ@¸Íi@Yùb¼c¿èõµ>:Î2¿Ûª7áî?µÖãÑ÷,¿Ï¢ô¡¨î¿âÏW xEŒ¿âAºÃ.¾AGNbcu3FGL J1033.4-50352MASS J10333216-5035287?ä2§-v?ÀÄ^©çCå?À~qÁsr¾?³j¦ÛêÑo?ζñˆNOl?¹Dt笓×?ãuùzÞòA?ÌTb'‰y?š;ÑùlU?¥•¹Øfš?×pOòB"¹?Êæã0J¸Ð?æ½g±ú1è?ª»"Xç?¶Ê³ð°'u?¡0™ñ[?É¥?¾÷%?¤îb¤-'?èʶP€?¬MT6""?•¯—)´ÅR?¢û±Þ‡?Í©ïð%Y?¬×vǐœ¥4FGL J1033.5+4221?ë['T>@M{À;×`RP.ìÀ=qZ¶.ü@!gضea?ô6%UúÞX?ç`^*WÂ?ÙzH0yÿ?òµ
œ;5@Žî
å÷¿ë}Õ]¿ù«¿çÄ£2Ÿ¿ì	ۂr?ÌêžÚK:'¿Å±ÓLBβ¿î÷#"úAGNbllGB6 J1033+4222?ïMÊu¡?"°8}ÜJ3?`øná
RÉ?`Aˆ"ô{?">xÕ*";?'ÂC8/±j?ïpÍ#†F?˜Zõü¬(µ?Píßrðpˆ?s*¥oç}?×}˜6G?•u¶)‰k?ì÷JàO^? ª'©M?";+qi;P?u"]a®ÊY?µ¾JÐ]²? /£%X­?ï{ža§yc?å°<g?"l®ŒDÚÌ?=¼ý51ú?gZmøJ?€ú˜íÎ	4FGL J1033.7+3708¿ïE]Ïõ@M¯Ž!–R½À:PêÔÑÀ<H™—ZÛ@»r‡[ÿ@bcQÞïå?®ì¿Uڗ¿±_2µ@3=¯÷¥@™£½‰ä¿Ý~7þÉõ¿éSFc'ŸÐ¿æȬŒ%=¿á¿ž{«¿Õ'‹Ã˜¾¿åTܛvékAGNbcuRX J1033.8+3708?ï
"c?!?˜¡¼P¹"¤?qÕ£{`?l?Oß[	?š:
ÕYUS?–™.ôeÑ?ïH¢kO(^?—‡ÏãµFØ?_Ÿ^êuÝ?zT<gÛ?"ó¸ ,Lþ?"õÝJº5?ÎOT?ŒU¾Ð—}.?nƒ|m§w?eË®C¯E½?¢ï»T9,‰?Šic'ýD?íéé_oÎ4?'"®Në>?"v_û(?vÕm?¢–?¬aq?Ýí?óÀ¾žß4FGL J1033.9+6050¿ïÁ«ãaþg@HŽé_ªŠƒÀ7åŸËmÀ;B`	UX@?6̛@ÚÝ0È?›'Z¦®?¸ÈºI½c@ g»/ìVÖ@æ­Øë¿¿Ñâb
a-¿Û'Ã'ë¿âøÎ}¦ôÌ¿ã[+硺¿æ~±='ˆ¿ë‹µ±÷	AGNFSRQ3FGL J1033.8+6051S4 1030+61?ï¦)>+ì¾?…hEm«Ô?R¯;€ÁÇ:?QιSiòÓ?"É엋?"(æh^?îç¤ß‹Ó‰?¥s=|F}?j"³è?|Ír¿.÷?ŸÈ³x#>ñ?¤ŠÐ¹²œ?îjÊ1ìù×?™ZIþçW+?"oÍUÚ
A?Õ §·?ž6ìl†·ì?bg¹ïW?îÛk™sx\?gM¶ímm?r°R1é?i·x	Ý8Œ?Ÿæ"ýzN?Ž–ì¾¥£'4FGL J1034.0-2547¿ã[­j(_<@;—s}¦À:å
55lÀ<[€¼S@P³`•'@úњ'ç?Ð?Ÿ}3\y?º4v͒?íA".ÎI¥@¡6Æ愿ìo—!Å!³?ïü4Ï¥©¿èÞ¿¾qjQ¿Õià»[¿ïÿÙiÍy¿ïù¯æ9AGNbcuPMN J1033-2544?îó­À¢d?Áè2ê?s^Tž/´?"ÖFŒ¢­h?œ²Èà_Æj?¾ÿOonQ0?ï›<\¦
5?‡+`;WP?Mî#7Ð+?a2ß_D<ç?‡R£ru?…O^µ¶Ào?î%HÔDyÞ?'Û÷FÛ?÷/º¢Û?vÂZWxǾ?©-¦ÍÚ?<ɲpy'?ï!©óډ?€ƒ®Ò?x;Y¡X9?h˜ºöYT?•¼	A\XË?|žhuQô4FGL J1035.1-0608¿Ì'ò*Õ@º@E•BB…À;$=Ìê)À<m"[tšÝ@yb|¡ç@cÄ*fÛ×?ƟEÀ~ŠÊ¿…T<S~"j?»3
nmñË@–Ÿ«Ÿ7¿ïÿDN
ª
?ïû—P=Ê¿ê$½Nª‡þ¿ä†ñ i,¿Ûèù¾_!¿ïÿ§ëkôEAGNbcuNVSS J103503-061204?ï¾pòJ½?'Üþ¤°W?d3Ͷ·?l"
|¸-]?v­÷sÆ4S?{4öXcî?ï Æ0d–?…ÝèÉfþ??²VCZ?PÅÞ+
«?†Ðá5í?Ð?"ÅH%Y¦|?íœ'dt¬?"úŠ8Z´O?Õ­¡—£?€ÆÎj£Ç?®õÔMWJ?o`ë?ï|É Ajô?v ¶
ûqm?eg!?…1Ò?[ÿ Ý)7ó?‹sϟÃ÷?sâ¦ø-[Â4FGL J1035.3-2050?߁àa©@?ÎA=·ñsÀ:Õ%¹Íì‡À<'ã'÷Ó@ø'ֈ¸@Á`Dä5Ÿ?ƌÇÀ'?¤>"cì'u?ß±cÚðÑå@ ª'¹V¿Ñí¼Øc¿êo4 ñ|¯¿àµ[–ÿ‹¿àæ €~®¿ègMoœ¿ïúÒ~½uAAGNbcu2MASS J10351532-2050261?ï>!1'º?''¦Øwk?Y¤EõF=?PÒ˙?–¡˜:yhr?'vMÉü"?ïžjv»ïÍ?'ºÜP™²?B϶Öó¹§?Q 9¬šù?‡8fã"ÑC?Ë¾RƒT³?âg—§?ŒA26þa?pUŽXÁK™?aèoÒ?¤›àn\1?ŠVëÕ7B?ï'ÿ&í¯º?{þT²2Z?g6ñØÂQÄ?R'"쎍/?˜<ç1¾s?z‰*ðp4FGL J1035.3+5541¿ïɢМ\@J4…]¢r†À:ÁœiW²nÀ<¤tæY@@ß-Ím²@-î4üa?Àqç£è§õ¿dÄòÅZ?¦ŠøŸ—3?ö±
Ô~ó?îM¹kzw¿æä£î‡1¸¿è,ðùÒ¿¿á€ðя¿ïÿ³^¼£à?ïò˜Ù€9vAGNbcu3FGL J1035.2+5545GB6 J1035+5542?ïÖWxš³?w"z'?h
T¸Ï?sꛯœí	?aԛ3K"n?`wҊylÓ?ìV.óÙ[Ç?·ŒÝh†É?šNÀ½x?¦ZÀQ.i?¶ºØ1ÕCÈ?°è»#Šä"?í/UÂwý?šUN	H{?"rE§y|?‡à«45O?±½(À'a¹?– KL½à?ìÆxÃÙC~?¤µÝ;Ç?¬·zÃÆË? ¼ÞÏÅn?¦ácG¨V?'µ`4FGL J1035.6+4409¿äf=\èõ@Lö¸–ž=À:ó­FÈBÀ<É	<¿¤@¾_°i¿·@1"œâú6?Á¾'cò¿eBØYØ?p?¡WÝ´>6?ø¥b¥?î©?~ðöοׅ–AöD•¿è¹ƒäün{¿äùAj-›D¿Ù°}ãۇ¿í€·_þsAGNbll7C 1032+4424?îå
Cõ¯?™Ç˜´S3ê?k£T'6ÿ?eˆç¹EÝÞ?ŸêT'#K?˜ÜŸp»ƒð?îªàäpp¢?žé¥A.?kžöÍ¿$Ë?qjû-v-ä?£˜L¨?Ó1êív?í2õéý¼?–ˆo5¯÷?"†r+zÖ?"¨/z
¿Ù?±†º…Ñ\¢?'áÁ-Dâ5?î)"Z?Ž—u¸ýÀ?—C¬1Ó¬*?…øÙGûÊ?£«¶€î?†èr¸ôgu4FGL J1036.2+2202?Ö4Dþë5¡@Mw™ÅXdÀ9ãíät‰?À<oîŒ:5†@Níd	K@¾€£ÿN)?³çØýî¾ö?©ëÿ~6"?ðüÛñ¨N@J‰)4?ɶ˜ØÔ¿çL?ÿIvÁ¿ç¯9>/H¿å'^!†ú¿ïÿ΢	?ïú²œ™AGNfsrqOL 256?ïðøí2>?XˆÄZ¥?DŠhø?BûI«ÛAÁ?SÈæV•Oë?RǓÿú"?ï›Xù¸}Ð?‹bI'}õ?Jôˆí…ô?`•
R…/?‡z	Q³š?ˆöw";"'?ïxç—?ƒ
W
Õ¢?sJÙùüº?e;ԊÚd?˜þ}ŒžN?<×¢u?ïñ8.÷L?M«ÛO…?F: $;f?=Z*Ìy›<?Rr'ÿ·ÛG?D¹¸:ç94FGL J1036.5+1231?™£glî@KŸ8ÅCkÀ;M♽«ÈÀ<È°­²UR@ ¯pÆf¬?ù ÛýÂ8?ßËlåÜhK?Ø6Ξ31[?üäª9$
ü?ôýìðƒ¶?èy¯†ßƒ¿Þ·";8?¿â¼g#û‡Ë¿ÁJùùUÁӿ煿ý±q'¿ï÷²ß:ãAGNbllTXS 1034+128?îuæ:á?¡=eªÍÈì?|xRы¹€?xÕSÉÏ?¥'n*·? `'ÌR(?ì]m¨am?¸UDé"G?Ÿ'ˆ|b©?­g"ßc'?µ3ôû¤J^?°-á¿ .?ìzÇN	Áü?¡%Vn'b?•
ýè©?‡×xr?¶çGÑõô?oÆ>/o?çùþ0Ù?¬"Øçۄ?£¥5_•V?¢*Uºšt?Ë.¹Û"¶c?«‹FŽâ{p4FGL J1036.6-3741?áFÁ!»@1äëÝ3L^À:ËƳ®ÖÀ<l$Ý/ @×è
Qé@½Ðæ7?у,$¡?Þ|7ž|ØC@Ó>ÿP3@§çC?¿©¶²"!7]¿Öš$‡¿ê¿>™Ä¿ì[1^Ƕ¿ïå¹,Ü×Ý¿äU?ÓªAGNfsrq3FGL J1037.4-3742PKS 1034-374?íò䲁"e?¨%(¤0•^?•ç%ºW¬y?'Ν6Q]J?¥Þ!ú»ãˆ?£×fÕ
®L?êù{|À6?¹G¹õ
?¯	Ðýl»?­¥ïYË?¸¯;ŒÇî?°2»\æ¢?ë5k1¶Z?¢"L¨ˆÄ?§÷ˆùRJ?']ôgJgÆ?ºXáõÍœ?›®fSê?êÒg›ËŽM?žÂ÷Ä/?³{'銝t?•R#xßR—?µñ18ð'?˜›IWC Ž4FGL J1037.0-1954?æ;É]	N@@g¿rq6¤À;‡p'°H2À<¶žõ#-,@ '÷øt›]@hwhiÏ?ÊØï…忘~º£³¦?ÑM>!MØ{?ù£²½'È?éµ8%á;¿Ø×Bœ‡µ–¿éÞ@\ça¤¿Æ·¿^û
'¿é [À7?Ý¥ãߍï—AGNbcu1RXS J103657.5-195432?î$ñý€¹÷?¡—'€T@š?ryBƒBc?i"Ïÿק?«pÿ£ø8?¡+Ì$ŸÒ«?î"Ò'
*?¡@ª
bÞ9?rÉÑcSý?1cnÏH?¤Y£aÎÒÖ?žôÉÂa?ínahøÄ?˜2 ³#»»?"âgc[T?z÷üAôZ?±ðª"ËÎp?–CÊš¦?ìYÓ7AA¥? H
}ƒa?.è†1öD?'Q'¦‹Ób?¹%¬$iuI?ž?½M-Œ4FGL J1037.4-2933?æHK¡û#3@8ß ù	kºÀ9º°"rÐÀ<MÝÙe@B†øXñ@0X<×÷£?¶4J4'æ?¤$§Õ?ì4"'òÜ+@äÁp‹?î<S£C^¿åiŸš´¿æ<m8è~Ú¿à»JùùU¿èŸó»NH¿êþøcSŒoAGNfsrq3FGL J1037.0-2934PKS 1034-293?ïÁº[?t§""ÏHÅ?VÔß¼¥?Kʺ¢¢TÒ?y=¹"?sÎ$Dì?ï·Õèôõý?$v1.Á?CFžº7"	?T|x"}?€Ö×ô?3QðM¢ß?ï._‹‰cÜ?~s	‰#üA?k…çÍ­?U
ƒ×¥w?–ÃQ«ã7?{qˆ0—Yï?ï›ÿÝøo?k©<G–?i•vÞš?R˕]&?'šÂ Š_ ?fŒó©šÜ"4FGL J1037.7-2822?ï¢ì¿äå@9äÚ<!~À8½ÔZ_ÇçÀ;°uÝÒ®Ž@4Ӕè@;7ÿJÎZ?¤[ã>?¸5™ióä"@oÄÖ^F@´·Ã{?¿ß3"À¼ž+¿á‹k~(Nÿ¿æn,Ε#é¿æ³¢.hž¿êx±ŒÕeù¿àšŠ?‰'ËAGNfsrq3FGL J1037.5-2821PKS B1035-281?ïÛUÀõO7?gÉÝѱoÿ?Oo9MËíß?IßªH}s?lÎp·=ÎÉ?epŠ'Äo"?+{ô?ƒ+OîØ?N;àc‡x?`2S7ã%e?…­÷h'v?ÌܛÙT2?î´iý*íF?'ÎgJ'?ƒ3`^kkš?~œsgiÁR?ŸÙ+l¡\?Œß,-‹?ïՄepP?`aۚ·¬_?PÊj"z?AÞÎAÜ?q6ZÂß6Ó?]ü§{&D4FGL J1037.7+5711?ᨣÐk@Iäh3Æ*À8óz¶ƒÀ;s¦#×þ@ψ¾Õé?ü 
¡©2"?›
ß"(¹?²n+Â%©Þ@MÙ<FØ,@ rIs'r?îø^ õ-"¿ÓÕ-¤(ï¿Üw®F¥¿ÙpÜÁ·oî¿Ý{C&E¿å½•!dԖAGNbll3FGL J1037.5+5711GB6 J1037+5711?ïål¡Y·1?c"ÞÉ%'?4æWÊè©?.'¯Î(gc?hÛOr(?bœŽš´È×?ïÈUÀ[?–]ˆ2ù$?f‡»·N—Û?qÿò3îÊ?š/~^!?"ô¸]3‰?ïPM/?ŽLªîK;?}õ	#åZ¤?"vߎ?•>ÚýM?†PzwšÞ÷?ï¡\,ì?†l8³ºk?q«_ç?c€_A?™!
¢~¬-?…a1rã~4FGL J1038.2-2425¿âô!Š"C@=BDËáëÀ:Ž¼ôµ4À<dêúµ=d@^ou®­Ó@E$Ý/?¿á•¦'`¿žó/{Ý_Ü?ÞbyœÏ3@4J5Ù*Ô¿ÏΧBy¢-¿ç nºu\¿âŒŒÀÃ)5¿ã ¸§{Úl¿åšŸ˜·¿ïûxçrjAGNbcu3FGL J1038.0-2425NVSS J103824-242355?ïÛX¯%?iAXu­P?Jo0CµC?A•€M¶%?n+?ô‹á?gOù~<2?ïºAn/Ån?4ÁÜ5ðÜ?8T 9'€ž?O–á Ö¿T?€­rBu?}=˜Y¯Ú?ï8…Âîq?|R	
á\u?hA>‹¥?WËàÌ­n»?•ç7V>]?yW·|'žo?ïž=:žkÝ?l,Xýôz?QUà߅Ó@??F6H…?†Eõ<tN7?kđ"¾4FGL J1038.5+3926¿ÔPœ mÄæ@Më¦ZÀ;Â:£À<éD=F²l@%¹r@¯;Ý%àd?͎àÃy¼Ú?²–ŸOwH?æ(ä$Ø&@Q-mÌaB?ïý÷Cõ"?ëg™6Jÿ¿æ9¸RÂD´¿áuú"pmP¿ïÿõEq#?ïÿ""ÆAGNbllNVSS J103845+392736?ïËD¡ªH?'Ó³jÎg?Si'''?kæ´ÖéM:?uƒN¤0vû?:±ŠQñ?ïc¤±%Ít?'<*¶YÖú?Xvx€'‡X?j…]:ƒ×'?'S=(þ?†GäÏ~?íi•i×?hF£LÇ?…[œ‡øC[?HTLJ:e?²á Hï:?›µ¸ÿû	 ?ïKønÉ0‡?'O¤¬áï?v¦Ê_ ?o©Í~¶Ó›?×ktB'?€1-ðaÝ4FGL J1038.8-5312?áOha×û@ž!S6Þ¹À8à@
²
ªÀ;<ý7Σg@j ñ@¿,0	³?³Åé?ˆâ?ÂMŒ¥ÀC}@¾ó
N7›@VÌ=…Ç€¿ÙXVñ?¿Üôï#¿èçóߋ@e¿ëfL€S¿ïý—¥£"¿à&OÀ1³×AGNfsrq3FGL J1038.9-5311MRC 1036-529?ï֞¥7úŒ?múÓqL?CðÞ½k"U?>Gúݨx?r2'ŒUHH?kÉú¬Ÿï%?ïE!6-?¢ôòeÎA?B¤ãĹ³?a{ŸüÅ?–ƸA,7ð?¢ÇHŽÁ­~?ìlûš7)?¢	·.åI~?œÃÿØZ"$?'
o£!çÒ?¸3˜-¾.?›ÌÿS§* ?ï܏<áú…?aš£ù##å?(FFí€l5?×%ÏtÎ?pö/W–¹ô?aH–ä˜4FGL J1039.2-2848?çУý(gÜ@9¹:'£À:Ý¢'vgÀ<5ZŠ[@ G5««@XE ›€ú?ǘÓv	F¦¿ƒXÄx{£?¹'FÀÙ¤w?åЏ"Ýó¿å›°å"?ïUG$¿ˆ¿çРa3÷~¿ãÃ?ñBοÝJSá)¿ËòEžÅ¨AGNbcuNVSS J103921-285009?îjºÓ}9?­~`–³‡%?qÛÏJ< ?u"ê¼¾?§3·NFñ?¬àÅ$›Ð?ìUéí±ö¡?·íŒU;?—Áäã–ëæ?¡ªK‰íu?·`7YŠ?²îuUˆbõ?ìVŸ}³rÿ?žõâ'R?'®²-àœ?†Mr?¤{?¸ßWXïØ?škÔÚ9Ëz?ãåH·~æE?®úðÒÈ2?±ÑüHümª?¢Íò±Þò?ÓÀï~Ã
?¯e"ôL&÷4FGL J1039.6+0535¿ìÀ²ß±@Iüj%™íÀ;(D9P"À<‹RË~îó@!È¿¡ëù?ÿ(¥ߙX?Ä‹ªà¿¿¬ÄŒü*S?élIŸ†B¥?ùð3§!lŒ¿êF~3⅜¿êIEßaô¿åÎ	Bžá¿ØYɟñ¢o¿ÚKXC
ñ¿À|•|ÔfõAGNbcuNVSS J103940+053608?ïÜrºŸ?–/-
xš?Tœž?5`?NnÅ/m0ç?§ÄÊø²?•°zÃ'¬?í°Ë4l¥¼?²!]#dÖ@?"ø曐D?š]´…Ï?¯µQ¢,?®1Ú
lœB?îTu11?1ÁÚŠ?rïÅÈ4j}?b2[*c,Î?¬ì¿ö_µ?ŽÝÆEeN?æTTǁ¨Ë?µ
áñqu?«w}ð'S?ˆ³2Þ=Ã?ÒLžù«ö?µÖœæ2eß4FGL J1039.9+7326¿íK…æoœV@DF~RvŠÀ:ÕüÍE˜'À<Œ>õßÎ@€®É"¾@µý}nÁ?ÄHGAˆ
¦?¦ý&Ô!¢?Ǥõ'Î{ù@W¹‹Ò[­?ïÿý²Gæ¿è7Æ´{G¿ç7"DZ£¿âÿ¤àõx¾¿ÝÀ‡å</[¿ç<V]çAGNbcu3FGL J1039.5+7324GB6 J1039+7326?ïv
>ãzî?‡â,´P'?J¨ù!"Ž°?Ag8­E?iZ"}Ñ?‡`÷–Ùâˆ?ïza²¹hL?‡:€¯P?D ¬e'?OŸ=èMV ?ÈûoÎ]?†z‹"Ɔ
?îªóÙ`£?ŒÍñIãP?k+5¾ã
?WxhÂ
—3?£­f{¼Ð?‹LMÔ¥h?îó2?'*?',¤éþŒ9?gzi˜Û?UÊé®N,r?žªuÀŠW?'KvëC¼4FGL J1040.5+0617¿Ü'ÀÁÚ3@JK¼'cÀ8®ìúi¾
À;éOâ–b­@'gÍï@ߢºª‹Y?¡­&ê$¡u?–¬þG»wÝ?ò'b`Ght@ЀÁÜXÜ?ïš	`ÑÑï¿âsù+Ðhc¿åf®à¨¡Ê¿ãùÓá>ó¿ä` Áìt¿îv¼àE¥|AGNbll3FGL J1040.4+0615GB6 J1040+0617?ïµÓ©
œ"?~¨™¹(%8?D
8bc?>…ÝÆ©eX?I¥eU;?}ÒÏ°«d?ïJN]ºx?†Å'Tx¦¬?G`s¸?WÞ¥X?Š·e7—†C?…?Æ$B?ïÆX!ôA?†´ûx)?qŽY0÷äý?d×X}rØ?›Cž¯ƒ~"?"ඐq(S?ïכ«B÷»?`û,€ž)!?Z½‡æ/›?N0¢PW$?k'.+N?YSáÇàÙ4FGL J1041.0+1342¿å¯
ß0@LcZ…‡"ÞÀ:åA—z©À<'šÎLÿ@ æã'áït?ùj;rœÕŽ?ÏSƒµ¬ ?Í2›ˆ²¼?þªYö›s?ÿT<xl·¿íO˜ß_vˆ¿ÖìaÝÀþ¿äCŒ?Å(ggÃ2Å¿çDÊ•Œo¿Ûdçî'CAGNbll3FGL J1040.8+13421RXS J104057.7+134216?îÅM·;Â?—3µ'ø?jÌaÎ?`)'Áq?¢'Æ3O?–_"yæý‡?ݲüX?Û<hRð?r'—ãŠ?zògÏ@?¢EAÑî]÷?šØy
xPª?ísž~6é?—"n:Š.?‡ŒkùO±%?x¢½s`Ö?±qŒäR‹?"\MGTª?êÕ@|\-'?£œÛg{­?•K.ÛkZ?Š@"ì>?˜3!éP?¢àç¸½4FGL J1041.1-1201¿á¯ºö>>@CÖî<³åÀ:Û·ìj÷ÆÀ<'á>sÙ@l^iAâù@‹QzF<?•5[×l8¿•õ¦4݂R?ӔÍí^<Ì@}禺¿?ïþòNf•`¿æ°ï@ëÁ¿ãøɪÙ\þ¿ÞBÀÄÖ´¿å/{]™c>¿ÄZÍÖâû7AGNbcu3FGL J1040.9-1205NVSS J104108-120332?ï@ø¥'?'ÌÑÑÐ̓?Y¶i3ç0ï?UºF'WG?–E"º¡+¼?á´Réì\?ï-2éɓ?'ŠçÝç_ä?WV®ÈWX?bå˜'Ô?˜í"7ÚH.?'@{ÖKãd?íü±'gó?'®Ò««\?y8ŗ}â_?c,
o×?­L:™Ä…?1YÛL{¢?îlûNzj?"¬öœôfl?xïO-´åa?aªÃHمþ?¦a9¼´?"§Åɂ4FGL J1041.3-6437?ë²£1ʏÀ¸"~–À:FU-XÿÀ;É'§
öc@æE'ƒ@U0 Y;Û?̉WW)Ýt?Í(˜zŠ¶@.QYŽç@Gì.'ãÃ?álÝÿ$7î¿ëz¥î;²^¿ÜN?=­Š'¿è©]&KÄ$¿èŒM€¼S¿ïÿøsCÄ{AGNbcuAT20G J104117-643103?ê´—?øe?¹"t€Ð?"äp¡|D>?~tÁ\S?ÃáZ˜èZ,?¹Îü1R?ÞJe°gG?Æo*í̐M?x›ó	ºî"?‡ê@‹5Xð?àÇ¢çV'?Æ3àŠj_?è4
VÂÆ¥?­ž¦_‡œ?ŸÉ^Lso?‰ùÀpÛ¾?ËOQy+Vý?ª2É?[§?ç"ÃÞê©æ?¦"n°Ê?Žü]òÂiÁ?xô­YÇÝ?Ͻ*¥)1Ì?¥ÝÎi'WÀ4FGL J1041.7+3902?œOrj;ï@NEž:WëÀ;&¹f¾zúÀ<í¬v0@ –$d
q?úµE\*£B?ÌEB;å?ÌHäu_þm@ˆô'@–Ó–•ƒ?í0G@0q¸¿á<Ybþä¿Üï|ÚÇm¿ÁvÀ{°¥¿åÎUÎh®?¿Ö² c¢¼®AGNbll3FGL J1041.8+3901B3 1038+392?ï#ÑS•5?ŠÝ=dÌtÃ?be(kKÓ?VmCá?™C(èB¯Ð?‰À7iŸ¯x?ïG| _ ¾??~ðÐÛ?Zk"'ë ó?ehõh¬\®?•i²ªÝ.P?È½,š©Ì?î
zs?'[Q1ˆ?|:¨Tìœ?juݤ5!°?«×Gé0Ì?âc@§þ?íÈ«ÜÌüû?'?ð,cäÛ?…ª°'ÌѪ?t¤~K€À®?®
–¼ûÕ?¢,‹!Ý4FGL J1041.9-0557¿ïTSaÚn)@F95" ¼8À:}ïunA&À<tރ®uÊ@ C?F'ß¼@y—=žÇ?µ]ÉòíÉ¿°Þ-mÉÝ?üTDZ±?ýƼT¯"½?ïþþ๿èL[B›Ûé¿ãÑ/"‡•¿àqýƔϿÜiµ©yŒ¿½¿¨L÷?AGNbll3FGL J1042.0-0557PMN J1042-0558?î'YõÎ¥I?ŸZ·Ý6-ž?m'á_x‹?bo¯ã}å?¥B$õ?žQ­J6ß?íx}/Ô¹?µÆÆFjÿó?"•U"ÿ­š?¦¨Ö'™'²?²žæÍÁnÏ?®Wjk%µ?튆n0´®?"ƒ¤¹')?€i&]u?luòì?±žœ©®«â?'Å4óør?çjî}È×?§Å†ÉÙŽ?©aãgŒ÷?˜ªÀNAÅ?Ì풾ùh?©oµÚµù¡4FGL J1042.1-4128¿ØZM˲@.Pð"aùðÀ:×Ûô‡ýÀ<u]9—@ Îvúmˆ?û38Vˆ¢Ñ?ÅÈqÞ¿"~?Ïm¿$˜'@È\$Ä?þÄ·ÕnݿՁ¤k.Í?ŽP:¿Õ¨#>ߏ¿ÀÃ*Œ›"U¿á¬!±€–¿èT5vÚQñAGNbll3FGL J1042.1-41261RXS J104204.1-412936?ì–V]º?²ZÜÊ%?™ÇÑFáê?'þ¥?ÕÔ?µPÀvò?±D°"Ÿ?ëåÇß!M?¸g<aþÖR?¡‹¬¥îiO?¦km¿PŽ€?¸ê´Xó?³¦$±D?ë½½ndÆ×?¢#!á0º? ¢]ãÀŒ?'ªÍ‹Ça5?¹Àåšùƒ3?š¸¼"«Y
?狦LúÖ¦?¤÷Q"çO?¶ËǃuW?lCkŒ¥{?Ækƒ
ZÀ?¡L¶¹(t4FGL J1042.9+0054¿îÀ+)¤i@HÄ$¢v·íÀ:½°}á­/À<qÈAíá@!º˜AÕ¸?ûÀ…`ýpÚ?ÄÍM¦&ð?­orÿ{ö›?étÀœ<â	@½±@Õ2¿ãЯgÏG¿Þå8Ô\ä¿Ý´	½#ã¿ÙyFÄܾ¿ÖÅl†;¿ÝÿePfËAGNbcuRBS 0895?îºR")˜?˜cG'œ|æ?]Y"z´Ÿ?u±eB?£qü™Ê?—"bd¤?ï'M–yç	?—£¨Î6‡Ï?RAŒZü?ZTîwŸUV?™ò4k"¯J?—4¿ß?OÂ?íÉ[ôޔ'?"Š>¦ÏÐ?uoVµYÓ?ažt¿Ÿß?°cYc 	-?'•Aî@œ:?ìR*O#¼?—jʧGS-?t)ЛÇ#9?eô½*€¯?¼,cÊoé?—•	#ó݌4FGL J1043.2+2408¿ÝD»»ÏÇ@NƒCc,CÀ9e"7ÉÀ<EÞ)ìb"@½×f"@_åÏÓ?¬6ÂZOy?ªÛ½ç'Ý?ú"Ô%†¢F@¬m™‹Ô¿Þh_ž¡¿àB1Ó·¢™¿åWøyùÁ"¿äÄÔævÁþ¿æ[¹™ê!q¿å÷]š
_AGNfsrq3FGL J1043.1+2407B2 1040+24A?ïNØ7àæ?Ì׃[ ?Tª
æÐ>"?P`tÛq!?"ÚX%'Y?*¹æÈ?ï~ڏ,Ýi?‹Ø2ï?ì?SDÝäÃÇ?c3ß$¥Ö%?àÀxH-D?‰'çB y?ï1"ÃñÚ,?›'ÆNí?j=…9…½&?\Z³afR?–…¶Ú"Õ?|/X•KÀã?þX[ù?pçŽBb¯'?sêñüæî?_Z¨.ÂèŸ?~¨•áÕ¡?gCîfNË4FGL J1043.6+0654¿ÙZ@G¾z@JÆБ}kfÀ;CT¸¾øÏÀ<¤lõÌ @ `Áïy&@#gÁLf?ÍBœGHéÔ?}ó0e7?²9Ž‰@?ÿižª%¿¹aǛ4¤L¿äPpZÛï¿éz¿8åz¿Ì¾MØü¿åb'q	¿¼öLWFŽAGNbllNVSS J104323+065307?ïіXÚV?"WÒ¤ö¼?S³ÚaœZ?Lë°ç()?*ŽÊï‰?"Ûå¦Ù²f?îÌR²b·¢?¡œr Ð#z?^SGð>Ã?hR{íü7Õ?¢H:šR"â?¡øécF—?íøKx?"mJi»™?u)wöþ?dì•`æÔÈ?­ÙÌc'Àh?'"ðv£s?íV¬Eö…Ò?"o÷"ÕŠ?|Ÿ=ec?lӎ¢Q¬Ž?³€©ùñûL?"—Úlí4FGL J1044.6+8053¿ïîÞøüß@A`»ÛãÁÀ9hùi
	ÔÀ;¶˜–dZó@ÓÕ)½"@'pOô4?²Ìx±—'?˼¤¡4™@'ÁC+λ@Ö»$,/¿±@}sž2¿ä(>ãjž¿ê×ÑÍmÜ¿ío±"‹c¿ïý"¶
+¿ï¤ÀßXÀ‹AGNfsrq3FGL J1044.4+8058S5 1039+81?î麦2%?¡̨¥.?žì¢$Àř?ŸÄú›%r?nàÕ3ǯ?u(ö²+øO?åø©æ(i?ËÆ¡V'?ÈQ"'v?ÆÊÝømC‰?¿˜ƒ¥GÑ?µâð	A@^?ëMlFŠç?©8ü;Dõ\?²,°uÏD? äõ:×zs?³gîø·Ù'?ŸE›kˆ,—?àùõK1žß?²*.KnV'?ÐS?ëa?´?bëIí®?Ëq¬Ë­Ã?±1piZ¼û4FGL J1045.3+2751¿ï²eîFo%@O
ÈuO7vÀ;<îM®ßÀ<¾TbWãí@ ÉýˆnU?ý÷¿¿ž!?ÅùcX¿ß©?o"=Äb™H?¨ÎI¾SÑþ@þߨF°"¿ïXPŽÌÝ?ïø]¿xÑM¿æ	°Š`A¿Û9ä<Õô>¿ÙiÝ^•a§¿ØÀäa>yAGNbllNVSS J104516+275136?ïæ"#ú Î?uÁ{^b@†?'…2†
©?&n""ʦ?hˆÝFÒ
?uj·¼ 9#?ï¬BÏʦD?"Ÿ³/öuª?=†FÙ?Q\½ýz?"cy$8(?ƒ´ÍîÀ|²?†>ã?‰íõÛ@r?i!4ÙÕ{ã?Thá•ó§³?¥Ò$NtwH?ˆ¼Ö4V?ïM)XqýZ?{›c`ê87?`}ôä?RoRgú¿?"Vã¶?{f¯žÑÝø4FGL J1045.8-2928¿éKS·¦ä @9éã%Ô¦À9ù=¾§pÀ<?
›dtõ@…|Þwïü@ý.^¸<?¹ýjúIݚ?¶™_·ö|?ú¥)ð"R@uÏCtžã?J¼¼´¿æl¸ N¿è	ò&ùi
¿ã!ý•Âu¿ïÿù_|è3?à
 ÒH7AGNfsrq3FGL J1045.7-2926PKS B1043-291?ïò÷"Ôr`?QÆ1`?AiÕVLÚm?>V¬oЁ?Q\Ï«ôυ?K'Þ5õ?ﲃïÊρ?†ej菀±?BºEDF+?VãH¤þ‰Â?'3_¹½º?"ßÞSA¼?ïPËí^³?'º:®ˆ?va¨ÄÖ Ì?kµ:Š‰?™|Q¡x?€†]Tëýv?ïây¿V?Z7n3°¨2?Ac?ؗ,?2ÇÉf/Û?i-péH¹á?XA3?¾P4FGL J1045.9-2331?ߝN&v@>úÓØYÈÉÀ:ãHÇïî:À<'âÐDP'@ðëzŒãÿ?ÿ.˜I7w?ÚÏyº×?×¹ügÅ?ý)–·g	ú@isyIm?ïÿˆ@«Áº¿èÑ–8W¿ÔâÜʶ¿êáôÃIk¿ç2Àç¼<\¿ïÿõž}.)AGNbcu3FGL J1045.5-2335NVSS J104603-232855?î}þ'7?¶g˜Tø«?X.=²2<9?V3'q¸CŸ?¦f®*Jý
?¶cX`Ñú¹?îÌÖhf>â?¡fDîs­?rÍ ՑÃ?ÿك>ró? Øøu_¾?›îŸ´Ø?ì‰äD"°?œ¢Õ©?š É8uÂ?Š‹¹£»2?µ.ÖãÍ?˜#Ï
}3?î:U¦þŸt?hñ_…?nG'$â[4?g"Ý{°.´?ªv-mÇã?GÙðÄXz4FGL J1046.0+5448¿ïAÇ~6ð5@Kǟfb5À;;u¨ùˆíÀ<ԆðI©—@#·&rZ@u砍©¡?ƝÁ¿@"…4õ?ˆõŸeÉÆ?ún5ZTà,?î'l^YR¿éŠ¼A9[@¿åäÌh"ÿ	¿è¤8>4îõ¿ÉúÙh<¿ïÿÿ&¦³AGNbcu7C 1043+5505?ïÁ¯á–ö?w%Çë@¸?RU0ä|¸?QDŸD±?z'Âû×Ö¢?v#´Ø?¼Ñ?î\|ô§ë?¤"î¬}þ?r·µµÒZ[?}mIé†?§áGùû6?¢¾ýJÜ?í†A:EF?"^¾'e§µ?‡5 ÿ«?J?zq+‡g¨?°çR
àg¨?''¯"‡¸A?îTUÿ
UÉ?¿yՃ9?c
øùþ?wËwÙU?¦aܑSe	?d‡âŸs4FGL J1046.8-2534?í®ÜøF«¿@=Y¦?šIÃÀ: ⴕžÀ<hHí¯›d@!V%–c.?ù½)Î/£?Èpà'ÒU?ʈÈ%ž:@hæŽ>ò"@7]kT¿éD,[Ø¿éýºÀÛ§Ü?͇ìH=o¿Ó—dá6¿Éø–T?È¿é"VœoAGNbll3FGL J1046.9-2531NVSS J104651-253547?îXÿ¼0dŸ?¡Š#ê\Ç1?qò¤rn?kúWT×ì?¨1¯¼÷g¾? Ä°:~‹?ï<NØqï?–k³UºÝž?UŠ_è½U?`÷([[?—~ÿ%–.?•¼~·R¹?ì®AŸÝö•?ž)^þõQ3?‰2ÒÛþ´ö?~\ùVïR?·g˜¥t¸?›™ï]–ß>?ìƒ#e""ð?›t$(
'?rḅ›€?f¾†8þôO?º¸ÉK
(L?šÞñ1Ò4FGL J1047.2-5517¿ïí¢µ}@+ $bµØÀ9Ÿj'E'À;]ûî"‡ê@u¤œ×è@'iߗª¬?Å­W¼w¯?§YÿáÞ=?ܕĢܹ@«ÙK=¿áÏ$Ã-è¿ç–¾¡¿å,¥3Ìá¿çŠü4µê¿ê$¼ãJ½"¿ïú
ÝÿzAGNbcuPMN J1047-5513?îƒ[
ä+‰? ls¾ÝH?U¢4=Pï?M9á˜Ø`)?§=¯ÑLê? p²tá'?샖Ï'`H?¾;,ÚàaQ?fÉÕë]í?Œ31aÓ>M?»,úÞ%¢Ö?½…†ñM¸m?éáç'l ?¨F¹ïþï?˜HL%b?ˆå¼Ïåt‡?ÅoYÝ­S'?¥Õ–SoÞz?í,G|
'?™Ðl±,ÿ?aUw*~?K_¨DOŸŒ?¶és›º¤?˜Ûôj
v¤4FGL J1047.7+7238¿î+qØàVl@Dþ<Q‡À9òOƒËÑûÀ<H‡Þ†2µ@¶;ÁÍ@UYΨo?¼grUx?½Y''b?üR¬9¯N@ÍÉæhE?ª)'þþUä?ï_]"Y
¸¿áµ¹À€Ž0¿âö'î½b¿æ?)@k*¿ãþ±·!jAGNbll3FGL J1047.6+7240GB6 J1047+7238?ïÓV¦'£?oú "^;L?QzÓA;È?IŽÇ/¯¶:?qöwøßÙ?l_¡†ò¹þ?ïŽí|'ëc?‡*oáID¤?Méĺ‹]ù?]ݕ
";?Šfœq?…t›êÌ]Ô?îúðނæ?ƒÐUÈã+m?qoö¤P†w?ekŒ3Ò±,?œE憫¡ª?¡HÙìù?ï^½,ã@d?x¡=N2äÅ?yVü¨G˜Ú?e®u‡<?‹¥6s'?tEée]'"4FGL J1047.8-6216?ïí»QÐ,SÀ*~#ûÀ8ŸüuÀ;$ї6èÊ@nâP3@2²|¿n??°ú¥Î\
?²—ºÇ<@Nõ üÐ@ª;£!¿Ì<Õ"oß¿áùbW
-¿çOÒ:Ê×)¿æáÑv¹¿åö8Öá"Å¿ïÿþ½à ¿AGNbcu3FGL J1047.8-6216PMN J1047-6217?ï¦J'Î4?'4pD}­~?EA]0É?C€2ԍ4¶?…hL?á†?·Òù?ëҎíÝb?½ò;ù8?Ní|ÈÖû?sê0±È?À–ÖËÃø¤?½åé"L?ë/8Þ'?§xC"mx†?˜4«ç@±ë?‰êÞSU`ð?À<‡
¥áb?¥¢uq¦ç
?í8'ã0¹?•©$C¡M`?'áiU¬?n—ªÈ°?³ãŽ>0÷b?•ÿp]Á4FGL J1047.9+0055¿ßƶKÅ@I:ÀÛ'À:n©ö/yÀ<?µÚBV@@«6$)U@U`"¥?Ãá!¾Ð?©9½;	kd?à½2?î,™@'ûF²Â?ïÀRÀí ¿ç…Þz¿æÊjåQ¿ë°R®"½š¿Ã"úÉ4g¿ïÿ$m'MAGNbcuTXS 1045+011?îí"i‹…²?¹ÉîÀúÞ5?wšŽj²<?œÀ9×gf?œu4Ý'?¶ éî`s5?ï2b~Ì@?›æs$é°?[tŽ
j?jý"`ã"?—ügEM¦˜?™]Ã	_ã?î–F³'¡?'ÓvÔîÓ?{a•ƒÜS?pÌS²hº?«JhäfJm?æš`aÍÈ?ïfEržÏÛ?{'TŸÉ»"?a¥	#'ñÛ?[ wÚ§­‡?'°‡µ¦c?zø±¼ð4FGL J1047.9-3738?àÜ^ËÅïA@3*ýڋÒÀ:ÛCîlYÅÀ<ˆU|3WE@!"':ûSž?û9JÚåª?Æ*ñÛ¥Ø?¹ûOìýD?öâý¹÷@îA~5»¿ïýš?[à|?ïáäVVMê¿ÛÚ胿¼ŸXö;¿âd.þ›&¿Ým ßôq×AGNbcu3FGL J1047.8-3737GALEXASC J104756.99-373730.1?ïÀ˜?†ß§?q¹'E¥l?CEƒ"ð£?8mŸÞp!Õ?}K/Ø27?p"èOçø?ï–L^8V"?ˆÂ|éÜú?NëºÜ|Ú?_F¢9©"Á?ˆ~,Ä"µÓ?†ßôO$"|?î45úqŠ?‹/ÙïÇՉ?t…V0Õk?bE ˜Â+?ª,'Ì°?‰oÓO-ÓØ?îprÃçQ?†aNI²°O?|Åp2àÅ?h·þ½¼€`?¥`0¡‹.Ì?"…܏h~4FGL J1048.0-1912¿îÔÛA.Él@Al½QðÀ:ùíp±CÀ<ƒCË0ëZ@†8sŽíï@ÞõfI
5?Ì}º•èŠ?À€È|)F?ñCâtÔ¾?û0£0œ*?ïÿì»"¿ÛÆDóO¿éÇ :ˆ¿ä/9ÿU5<¿ã¦ YžØ¿ïÿÿ" 5•AGNfsrqPKS 1045-18?ï‰,e;Û»?‰'H͗?`Z*_±Ï?_½J2(¾!?‰ž\±$‡?‡tW $®m?ísj@NZB?®Ó:šD"??z5á?˜áõޚÍ?°uk6ìëy?¦}Ù:ñÀ?ì÷BH8q?š›ÄÄ)J?'3'ä¼?"^óQôè?³¹	ن•k?–&xoXÚ?ëú\CÎö$?š+Ò'*·Ž?ŸÀf!ÝÐ?‰ô¦ÆK6?¸g­Çÿ×u?–vŒ‹
ÙÀ4FGL J1048.4+7143¿íûqºFQ7@E$	_$RÆÀ7"
ƒÁÀ;4òtý@/öU²9#@ ;>šo'?ÈîN…QÂ?µÂ¡"~–@&0¼Y¸:@!áªqKµ¿ïÿÚáb†¿ê[y£Z¼?ïî.¡©¡?ۜ@]=Gß¿àLZK¥ñ¿É¢
cAïAGNFSRQ3FGL J1048.4+7144S5 1044+71?íúܕ*5Å?Ç1Cѧ@Ú?z[›ÍoÅ?¨ïn|}?­Ã3¹Uµ?Äý¢±íà?ï%Èè&? ØDŽly?mÀNàÆoN?…À­±v‡?—ŽÙ#¥Mi?žmÞ,£?ìmÚ?.(?¥©&•
ŠÏ?¢:nËö¿?šŎpp?³yáÈe?¢pGDÉâI?ïüo²h˜ë?B(¨Y)E'?
²m+–?'m šÓôÿ?9,×Ú?@ïÄ¸|4FGL J1049.5+1548¿äÎXGa4ñ@MÉrGE8ïÀ9ï`sÞ.À<_þ99@I6ù;jº@$ù´Œ?¹äÖÙÀü	?¶‡ÑßÊð?úd§՟Ú@V'+áÛ'¿ä­òˆH8¿äJúú¿àc^Caÿ¿ãmó=yÞ¿ê´RbM}¿ßä«üƊAGNbll3FGL J1049.7+1548GB6 J1049+1548?íã¿|sD?£‰3åÏ'?ýºvË3?uä!uÞ$5?­D™›I(ì?¢†<ÎîÑ¡?ï– ä¥?–Ž5ϟÖ6?j?T
üѦ?u"$'ìJ?šÅQbµÌ?"ïVÓ\?í¾µk†¿"?˜^tàñ½?Æ"ãÇY?ˆÆ'+jîå?«±—Õ°Š1?'%È"'×?íÞØÀºy?'Ê܇ÃÄÝ?—bÂWé­?€oá
u‡?¦m±jÈc ?‹ã|§E
4FGL J1049.7+5011¿í¨§œš2¤@L¨6m
JÀ:îÂfA}yÀ<Õ? §?u@圧k@ÂeŽÐ?É7ôãí$Ü?ΏH\æ
?þJ†_¡P@é¶H¦âØ?îrò yI¿ãÊ\º³¿àd¸aý–¿æMzV[V¿ëoýV'n?Åb¸ÜÕÙfAGNbllNVSS J104857+500943?ëôé¥4Á?²
_ï««?LÉ'¸?…íªëôok?¼¯?F?±!åƒxÇç?î`¼Õqâ?¢»¬úi–?t'/D]¦?{¯À¸¨?§cìÀV=š?¡–r5X?ì޴Ќ¦È?žhaµá:Þ?˜š¡"%;?Š
Á-:?²ã±3t?—¨Ù ¬?îlâ'ZÂ?‹"w¶-É?Œ1´S¾?tÁš†^§?¢%–]CC
?†üî<i•4FGL J1049.8+1429¿²‰äÚÈ~ƒ@M'bS—WÀ9LwH5ù·À<2¾Ÿã_¶@q*EÎÁD@kÉÚª"?®žˆýÑ7Ò?²=ïN×Ôh@K¡F6E6@Ê
¥/$¿l{É:Ç¿ä«QݘL¿æ¯Õ`EK¿éœÀË6ʗ¿ð?ïþËÌÍAGNbcu3FGL J1049.8+1425MG1 J104945+1429?ïð"ãªÿ‰?XòÆ;yA?9tÜZp?3"ß¹S²?X¯[¨IÕ6?V†Sà6ú?ï=»aே?¡k¸€ª?g†ˆŸŠ¹Ã?†{Sj6?•W¯ø·à?™}|>¨ø?îñ©þk'?ˆ(·'':¼?y9MՁŽ€?uý~dßÉã?›|‹êÒ*?…7÷ʉ·?ïÇñEøï\?kÉeW4‰?iœÀÛ¨ª¸?b¯øY?nqù+gù{?`GõRtá&4FGL J1050.1+0432?ëþ{'Ï @J¨Ü]cˆfÀ9UóU͒À<,	óžÉ@Yø6zæ@uƒž?°‡ÇŸ'UR?³óÛÚ[×?þœÃk$;@£3ž¿Ý%#:—«ƒ¿åâ1ž½d¿æwKüWÔÓ¿ê\ÞCÖ¿çŽR"_¿ïþ‹ Z›AGNfsrq3FGL J1050.4+0435MG1 J105009+0433?ïù¯>S?HÇs3W?#¯1%à´§?&n$áç?Fñv¾z‡L?FÄêP×:t?ï©ßÑk"?‡k׬ޑÝ?B7|/Tˆ?XѤ(·µ?"d"õò)©?†ˆŽ.BÖ¶?ïCÂr§›Ñ?z¯·‡^	½?k"r.?`Ö÷Ï2?"#_Èk÷›?wМp5ð`?ïøˆÌóÇ??o"etZ?0ŸŒ­'?#²lY?G®ê
?:畫Q7Ê4FGL J1051.2-6517¿Ê/1¯-2FÀ0¹~;oBÀ9l™ÝŒ7±À;·ÊX~F@"ýûÃÛ7@ÛØ{V¸s?´£è}ˆk?ªœ©!)£ñ?ô‹'æÎ×?ô
ôÀéú¿Ò.žÎ⧿Ö*èÁŸòú¿çм{Eñ|¿å¸/A8¿á¥Æ}þ2 ¿è"ó!uE§AGNbcu3FGL J1051.5-6517PKS 1049-650?އ'ː±?¿§ñ†Lƒ?'PS¬)â.?"/|¾7G?à1³üÖ¡?À!'´ÿÖ?Ï£>¥
òç?Äl(à@{? 9§Và[?¥å3å{‹e?ç•æ‡A?ÅLxWF7?â®?#ŸA?°$NÒ	Ð?¨fè¼3?‹@)瞌Ê?ז¤¢Y?­ªqA?Ý
‡«Ù3?¯õÔ	0ø­?ÂaŸÇ††?¥ œÆ–ÓÇ?ÙÁ¨šã¿?®¾ñ¹®Ê4FGL J1051.4-3139?½$ùšÇRK@8¡¢¤Û<À:žpÆ;¹À<OÚy]¹ï@ÿ·1Ô@LaÿÏ?Þ'_Tú-X?ïü«ë«µ@ BÛ@ í‹^B¿à‹ÛÀÛ|é¿æ(bÙ	¿ìÓ¤¢š¿è9ê™w5¿ÀÄbÛlwÍ¿àöÿ¦=ìËAGNfsrqPKS 1048-313?ëJìڟ޹?ÉÒð]}T?Á
®¥^Õô?ɺRìz
?Œ™ßò\? 6v®j¿«?ã…˨j@?ѵ/ôÛ?Ò5¨8'?Ñ>çæö¼?ºûÝ"È?²ä&rLÃú?ë,鍕"?¢õÁtdW[?¤ü]Lr.z?"zۆA?¼"ðê<?ž•
giæ?å̒²0?Åê&Õó€?ÍöL‡¨‹?ÅØ˂Ž?µ®ÒF7õf?´Ÿõ‡Ó\Y4FGL J1051.4+3942¿èe±s½@OS?B5/À:Ò ùtÌÀ<'Ejm\$@!&Ö>°!?ù•¸~a.ï?Ä®j·ù?¼x`äÇ??úa…Æ}þ@B·¼Dif?ï÷"ÁpME¿è!œÓ	ý°?ƐöGo€A¿ä‰6?W-ä?±Ú, ‹À¿Ú"þPÅAGNbll3FGL J1051.4+3941RBS 0909?î ¤a3ò?®<˜Nƒ?^4•lç‰?x³6o@vq?­F9Y"?­Çm"FÎÚ?ï.7mƒU?˜«Ñ‰§G1?WÖ0¹e?dÔéa$œ¾?˜»¯NC±?—ŠñùÒ?ìåýÿú[ï?£ƒ¨+ µ?m0QlØ?aß\ÅêZ?·æw¹¹¿?£T]ÿ›?íÍC¼Ÿ¡?—ÛÉ6`‹?\ˆá‰˜£?W+r&΂|?±%*[ô¢Ã?—¡ì.Ɖ4FGL J1051.6+2109?×1HîT@O
üçFÌÀ:Œ@O{hVÀ<Z)ôÆ@èåtc+?ýy*GÒ'?ÚÉLÅUŠ ?îâÁ*Øß@ã*!;¹ê@´ÏüØ`¿è³pÛ4n¿â.	È֞¿êqN õC¿ï£GÞ#¿ïLZUÕõ¿ënƒÁ@&·AGNfsrqOL 282?íIB|ö;À?¹
Ñ7a_?`Ï(Š'Ìr?e"ßVKð'?µ/rÓüã§?¸ÝTÃÒ?í@ò€qsŠ?¾Ë_Œ·(?ž)ó\l´?±¯=i5'{?¬ÛÞJ²m^?±jÊ9µ¥?êڇn¤Ñû?¤]‡Ž?£k7b׆?á<µ"ZÅ?¿v(Ùm­?¡"Üoç})?îIÂ×?—yj¯=?€o)å?¸"w®^á?£Ïœ›'6?"ìOJG6i4FGL J1051.9+0103?ÛfÄ|"œ@I¢pÁ3;—À:¨ÓÚGóÀ<zµ'»@ "~/Zá?ûÔ¶:º2?Éž–Xœy?ÊÁG3@nÙ8@ Þò¿%¿î^&@Üi"¿Â'Š^h@0¿ÔHÀc1þ€¿¶[Ø}Z¿ì\'Á3¤?ÀÅ`‡TG«AGNbll3FGL J1051.8+0105NVSS J105151+010312?í´Þõ_ù¤?§†ÌÑ?=)™vÒ?zûšµ S?°1c!Þ
?¥ˆ/îr•ê?ï?wÃFÀö?•l|æK[?a‹Á5\P¥?q\—n{Q?•ßp|W?'S}QKþ?ì«Î‰?™áò²ò
?˜!–!¡bO?Š[á6Š¡ ?²'Ý"93?"Õ°ˆg?VÂ?Ž]ق"o~?…¿‰'š¬?uÌ«ý_Â3?¨¯Ç(:í+?ŠK~î႔4FGL J1052.3+0818¿åáKŃàÓ@L.‹*kÀ;(Ï,"žÀ<€w˜½Ñ‡@éª{i,ê@‰$y\p?ÉÔ®ƒ
¶è?ŠÉ'"C
?¼"•£Àº@>%ühñ±?Á©p¨	¿éº¼"pdí¿Ù·áéÏ¿êÉÞÛÃ
¿Äpjá C'¿ïÜè‹+BAGNbcu3FGL J1052.0+08162MASX J10522451+0814095?î4s/÷š?©d| ­#å?ic¾¯pF?f²HÊݜÖ?«'ěhý?©	ý7~}n?ïPU€âï?™)ÿÿür?Oþ-(ïY?c'K¥ˆ|?"õ^"#¤?—»(âM?îVŽî|?"ÕéAïٛ?z
‹3#r?s®'ˆ?ä™?¬™V?±Ú(?'ÉJŽ2-?ï…mˆV,?t¿É=Á¾?B"ƒŠ?=…Á	?{\¢<à1?tX|óÃû4FGL J1052.9-3743¿Ù/Ÿ°4Ò@3r§›ºÜ
À:ŒPx¾W¿À<|ÏÓèJ@ U*Ï?ÿI¦Wíþ?Áå'Ác?°JCp?7?óec>"º@,ŽTÁù4?íº|CG}¿ÀßsXd¿äµ¿Ý…*¡¿,ü¿Ð?›PÔ¿ë.
ß¼"šAGNbll3FGL J1052.8-3741PMN J1053-3743?î±	᪊ž?"þ_ĸâ?t¨©±)ÈZ?mñ÷'7,?¢ZL¯2?"8E{\W?ï@²Ž¢Œ?nÝ3¸2š?TÁð¬‰m¬?aÞ¥ûT&o?–¡Ê£cÎ?Ž;""snƒ?íäFô‡·ã?'¾
—ò??|á®Ê¹?gƒ,Ã#{=?®8¬ûN¨k?@BÇ¿¹?푀<'˜?Žå@jã,?"Je¼Ã(•?q»ÐèÔ¾?°ê±dR®?ÿ½IÛ4FGL J1053.7+4930¿ïÿä#«€Í@MEhÀ:´ñä´JÀ<m¶
éh@nˆcf?þ/}0­Fö?²ë¯α?žn"h¶?ìܲÞd#ì@.ø3
ò?' Wú?Ê
áÄÚ¿âd…†"¿Ýýc˜€À¿ä&@×`¥?º>¤@¼;AGNbll3FGL J1053.7+4929GB6 J1053+4930?凜˜éaÊ?":¼'Àä5?LKí`Ÿô?A¿'I
b¤?"Ö)VуT?ƒëyŽ9o?ïrh|–ý?"[:Í®•j?QØcû?]‡í•=èZ?¢ošV?']/X՗™?ƳÄà?‹h»Ö#ã?oÄ¡e)ŠA?k'T«)?£¹~qO?Šr¬T"|?î'h¸vÔ:?‡çsK&ò?‹T	²'‰@?sÀ‹ÙNò? rÚ?ƒŒI*Ó;‹4FGL J1053.9+8628?çÑàAF@>0)à¤&À;7Žd²1@À<Œ†ÿc"@ =ºßd@W#"ú?ÆN­øvHÝ¿ˆGQ€Ù·Ê?Á<×xLm@(W$T9¿ïwWÂHå?í	ۂr¿ëx¤ Üš¿×ë'D"Wá¿Ï
W–꽤¿á#=Qš&‡AGNbcuWN B1046.1+8645?îµÕ€+á?§šJãƒ?fè#K(^)?fÁ°"V5º?£4,#J¼?¦Î\¶•rÐ?ï¤v¯ÓË/?"G/Ù5h?@?°ê–Û?P™Ä@€?…ÞXüez?ƒA…<áÕ?í ³ÔÅê`?–ŠÇφƒ?z*ä"w/?h*À'B²?±W³•?•ò.Ÿ³?ï6ÒÌÁ?ƒÐI]ò«?ká!øWí\?aÀtDþ?›ýgqª?ƒA˜î/Œ+4FGL J1054.2+3926¿ìp4c	Ç@O`ïܜM©À;Ê;"À<±ákÀB{@&a"ðh@h·¼šO¢?Ô	éã³ï?Ø*Ov`@ÇMœk2@J‰äDãŠ?ïì,CTéf?á£ÂýÁy¿â° ¬³R¿äiêIµU¸¿ïü`¾†¸ì¿é'kb#¶"AGNbcuCRATES J105433+392803?í³/öÅô¢?¥_Bۗc7?™s£êÃ*?'ó—‡Lñ_?¨vÁ«T??¡X"?êS";¶'?¼	ƒîzÊT?²fnE…~?²Þc1]ì?»XyoÜÅý?°[š×u{ù?è÷֛͉;?©çö–[k?µC…å/<š?›n->ã??Á~âž2<Å?¢Sy3vÁ?åœ%Œ^O?²‰¾¹¶É?ÅÉœàÓ?±ì'§ä8f?à ›Ìîkï?¥»™°\ 4FGL J1054.5+2211¿ïf¹r|õ@O…" ä¶À9s€*]À<ò³ç#@,4XÍ@¼{ٕ2,?©?Ï£Á»¢?§S›2 ç?ü½CŠU@ÕàòŸ?ïû)×iß¿áón!EÊå¿â88 þ¿áI™;¥È|¿ä5D௭­¿äáü>ª_ºAGNbll3FGL J1054.5+221087GB 105148.6+222705?ïüAªæ-?v,'Óf'Ø?Cs]¢w™?:¶Ö†Á@õ?{³{^ؚï?uQ5·»0?ïC4õŸÉT?"L}vÕ£'?aòŠ¾'û?pŸêQmè?•yBú¯?'Vå°ó?ï,QœG—?"9-Ó?jZ¿µ°ì?YmGÜ6«?—*t–èvì?|cZGØÄU?îšÔ5ôê?ŽÈ83Ža?'–wi<½?†Ì|0bÔ?šªïØ&:?"÷dÙA%ø4FGL J1055.5-0125¿ë¥0_)—d@I
ÅÁ?ÐÐÀ:G­§m—³À<OÏôŸy­@ >è{~ü_?ÿ‡ÚTtÌ?º›äbÈ¿ŸZ|Î1Ñ´?ä¥	Œ³@@"¯Ò–¿Ãòæ&¨¿ëù@€¿ÇK	ÿ\–¿Þ|_p#¿áb¡ N>§¿½@Y6}©AGNbllRX J1055.5-0126?îÁ ü5Ã_?¦{ö¡ˆÀ¤?q[ŽÀøY)?c'Jw4á²?¡Â~d"¾ó?¦UÆ5"t?îú¿ÒÏ
‹?œÏ &©Pô?[>±å~X?d²Ðs҆'?žöñºÿöÐ?›ÕHÙÅp ?홁+ø³j?'ä¾·îî?~î0c÷AB?l'mìl?±E™úð¢?'CëºÙÚ?ìÇØ/MhÙ?"ÓÉÒVh?©½) ގ?o]Q±£T?·Œàpm?"2O&Šª4FGL J1056.0+0253¿àT›
»xo@J£þ¬BêÀ;–(Ÿ~¶À<­¸6<Òï@#U´D•±-?÷UGZ1¥?Ð[j‰á•²?«™lÈ?Þ6B\Eü?ý¹U̐<?ë~·–ã?"(H7k?íjcì8¢ß?Ôìi ,°¸¿Ýê!;¹êr?Z9¡%BôAGNbllRX J1056.1+0252?ïnëhQ¼z?‡Z¨Àe¨u?E<Â?­š?<ƒg•€(¬?'x¬å¦s?†ø6]5Ÿ'?ï °¤µ;?Ÿº÷$ãîô?WÑeRœ?eÄÛ?Þç?šxË<GƒX?žÂ8í—S"?í¹
ˆoÝö?"®©_'õ?u´}™òJ?d'͆Å?°ÜKâáð0?"Ô'=Þ§Ù?ëÿÞXÚL8?«3mxØeò?w29؜ñ?sùS=œ·?¾ãet?«9ޅ¡^æ4FGL J1056.8+7012¿ä"ø| [ø@EôÚ<÷À9,azn['À:§9zu$@TdhµK&@Y£ÙŽ|?¿¯Ý'ãɾ?½*Œªü@	Ì΢âa@ÑD]'""?ؗ,¢z¿áø"»ìª¹¿è³Œdþ¿èžaŸ­.ø¿ìa‡"à¿ïý¥ýÖ.AGNfsrq3FGL J1058.1+7010S5 1053+70?ïË-ê'?©Lg4|*?y¹ë§ËO÷?§C»¢?–xrÛà?•'"U×É?ï;BD+ï ?¢Š%¡Þ½?bÕ,°eLÒ?}ÂÅâ?–=äub^? ×xÆÊâ?è­)Y"&?°~
?}¸¡?£ñ!_$?•4šm§û?ÈOWž˜?®<ÊPä?èӉ…i¤°?µGJHõܨ?kãÅ3rŠà?aäÄ\+EŸ?ÌBJՋ£?µ-C	²q4FGL J1057.2+5510?é?'ì
Þ3@K"£½ßÊÀ;7='¨»À<á±¾SF@!-ÒK;é?óT5€ëM?ã9û¤P­?יG¤¯L^?û"üa'@˪ZÜð[¿íÂÎ{ùu¢?ä?°¿í#è§ô¦0?ÝWH…Ö¿Û'îM®ß¿êP
¤ž°ZAGNbcuSDSS J105707.47+551032.2?a5}z?‡ôå*ù_"?Púêmç}?M^Ù(¶Ïð?}憧" ?‡ =žGð?ï§6Z™\?…ñ"ÌOgÆ?C¹n/¤?_ä&˜g;?…­ÂÙxÓ?ƒÈH87
?íï`Þôu?"AÅHÇéE?~ÝÞ5•?pc"i–?­KþO´ñô?'NÓD±§õ?ïÔP4y¥Û?f5.7mn³?4å?å¶ÜJ?IÙ#a'¡?t‰'ÄѤ½?dûô†§t&4FGL J1057.3-2341¿³1öÔ$ˆ@@ó.ZÀ9ã3cښìÀ<PÕ˨à@+³ß•ý-@SEø1Õ?»Ñá߃ˆ¶?ϙ‹Và·@r:½k/ú@Ü¥!âþ½¿ØHˆÚځ–¿Ú¬Cà‡¿äû…LXž¿é¼­?"¾¹¿é?#âqŽ¿ïÿס<%JAGNfsrq3FGL J1057.3-2341PKS B1054-234?î|ޓ/?¡ç,Óù,?ô…'à®?‰µ…N
 ? ´õjüâ?›mŠmèí*?îùPÇuHŽ?™[<ù"*l?t`­gÒº´?Â6¹j¤?›½»·b?s?"_c2ÀÄ?î¤ÑVZ?Ž³Ò¾?'­v‰[ù]?wÛØý Ú?¡Œõ¸ü?ˆ£KÛh"Í?î|/À;?‡V£õPWˆ?"]-Ä¡!?{{ÇkDÁ@?œ qõfi`?~:ÍðJћ4FGL J1057.8-2754¿á)'õ	@<•ŸÓo~=À9ùhG6‰À<BÃú–3´@ }'Ñ#I?ý"VÁ­´Ú?¸cfAR…´?®3Øþ?ö"æ™ýl¨@ WمÂÍ?ÑÀ&€ó/¿Þ=¡`¸Q–¿ß³þ4Måf¿ÒõJd¨ E¿æõ2F¤)@¿«ÀÀ9ÁAGNbll3FGL J1057.6-2754RX J1057.8-2753?4Mõ?wÝ2[yã_?R#p…€?CV7làüÎ?†XØÄÛÞ?vËYÁ"#ø?ï"^3Â&Ê?Š"Á…ì[?Rݨ1(­ ?b¶XP]?ŒŒ¾	Q7¸?‡àbÉ7ð?îÖ¨¤ ä?"rŠÎ…¬Y?mëå@­?^®n'Ì"? ¶¿á´†ï?ƒ(̝';p?îõö.À[?‡'"ê ?'®h'X?eß+Íâ¬?ªºõ
$]?…ƒBÅBb«4FGL J1058.0+4305?à‡?ñ¨ò@O	V"À;Q4‡Ç	>À<ÔLR¾éµ@ÞÑrMû6@'¾´V?Áø­æ­ž‰¿«þym)N-?ê…¸Qì@	?Òñô¿ïãåÌÞÀ?ïÛ_W5¿é¦n£¿é~T>p©
¿bÜ­>‰u¿à¿Ýƒ(iAGNbllB3 1055+433?ïЪõ'8?}ü[ž?P»¼íœÅ?Yù7"^R?s{•û|õï?yg±ø¶´?ï¹Û&« ê?ƒ/o|Áû€?>'²uã?UÄ:Úr¹Ê?€"¨ÄþÉî?'Ìÿ¹Ç?îœÝÌf¼\?	ë-
{?v"ßÎ'ä?tí.Äbœˆ?£mÇ?ÏYæ?ÂmòÓý?ïç.…îx?Wì^†?8±$V¤¿?7çv{Ú]b?e»Vl&´?V5êj¹ød4FGL J1058.4+0133?ïqãùD@JbëÝ3L^À7æR¯Ð=À;0;pïVe@À'D@…›"/Õ±?"rºÝŒ¾?¨¥ã»@'»=XP#@ÄaՈ¿ ªÆ©¿áw¾þX
¿ä'Þ^ð{S¿ã³'i#°¿åc(X䝤¿ç&ÆsxAGNBLL3FGL J1058.5+01334C +01.28?ïÇ,_– ?uìçŽ)à?A‡j\ø]•??8%'j?z8âí•å?tQ»¤Ì[ß?ïf$"?™"(2+?h…w{\ê??uÌ$Ó»Ey?™,ðO?—™zöY³Þ?ïL7Ý2‰?†üÚ°l?w95)S4?vÿ€©'?ªØ—Z?'\AüYd?ïºÞZ¶q?lRtt i‰?]ñÍ›9™?RQ[C›°Ö?{zŒ=øÎ?iL8éf~Ï4FGL J1058.5+8115¿å.7ö¼_@A_ d#–À9ÃÁ>#Q>À<¸Îé@'<ýâC'@÷¯~Þ,q?º °å¹±?Á¤Ÿ\&G?øQGñ0Yd@CäýÆö¿Þp*
ag¿æ5deÛ&¿æ€\a)惿äJ¯@ŸØM¿èæt¾˜×}¿ïóÓl#>ÉAGNfsrq3FGL J1058.4+8112S5 1053+81?ïÍoOñØ?{
$t|?TB´³›ˆ?TFå:3ÚÂ?t7њK,ï?w÷±	ò4Î?ï®FbOU?'"{ ^ÑY?<|ýÿ/³¯?PzÂ%P¹?ƒŠs÷r­?HÒéBáÝ?ï,â®Ã9?€P@âò ?p.ƒy³‡?b¨VK½ÿ?–bÁÉI+û?{«õýasê?ïˆûi¶rZ?tpÖèàâq?`'4ƒÙ:?J—³»vL¾?‰œ˜qž³?s†m…"4FGL J1058.6+2817¿ë}ú"†4b@PCƒQX¸(À:%W¨]'À<vÄÀ§%@É{'G•Á@˜>{?´©8ÈôP?£×¡çñÁN?í²"\KZq@X¡C§¿ä|)±ª1—¿×ºÈ"W¿ä±õ桊)¿åñìa<°à¿â3͌æ-¿ä¥\{¬AGNbllGB6 J1058+2817?ïš'M,Yg?‰ø'í½ð?IÍÌñÂ?G@#w¨ˆ¼?‡ÙT¸"z?‰V¼ߺ?ï³
vTäT?ƒdòv…ô?=£òq;·
?Pw+ºNr?'O'×=
&?'y'ÖÁG³?ï§Û*·?ƒ±|'ék8?pyò£_Ô?bûÞæyu?™L¢ÛÂÅ*?pòÔàï?ï¾DDøÇ?fLß'«?Y]6…D5µ?Eí§üóž¨?z†â¡Ø?dے0 ó.4FGL J1058.6-8003¿ìßµ~ÜnÀ2IêþæûLÀ8Òfàß©HÀ;ËûSÈÕ@<'UÓF@ö@×`¥?§Ã¾s?ÂÆ'De
@0¢_:ù@½r,mFT?áÀ½šTÕ¿Ðâî![Dt¿â֓ n¿ä‡âT1¿é|õSԓk¿ìð"rϏAGNbll3FGL J1058.5-8003PKS 1057-79?ï/àTF"Ø?\I Àï?u÷ü²A?u
q>œ?"Â÷xÝ7?‰ÖÙ¡S²?ïÀuž?:gc=â3?AWÕM!?[	¾aŠãk?}¥m¶G"î?€Bî—L?ìÀðå†>t?£PBö}Ÿ?§jÍ"˜Ÿ5?š•ó
UL?¬†$…yˆ?˜_è'Ö?ïŠCeµx?t‰¼MB²?]•8ƒK©‡?OB%Ùâ¢â?‰¼'8†î?s3q
ãÜ4FGL J1058.6+5627?×!{»7N @K7Y‰ßsÀ8+È5ŽWFÀ;‹ïXèÏb@B_ úa?ý¹"vD)û?šÀÜÿtê¹?§t®R¹5k@IÄ|œ2Ñ@§'ˆÛu¿Ð'¾^"¿Ür´þNúå¿ÝظG¿Ý…bÀi'¿âPÝèþÝ¿ÚbNAGNBLL3FGL J1058.6+5627TXS 1055+567?ïÐGúd	†?qáOŒ	Ö?(ò©;Áµ´?#>T}Ջg?wm"0Q?q¦.«Ós/?ïpŸ?×o?»ZÂtv?R{ØÂóñ?bÂ:'õú?ÕŽ‹ãS?Doè?ï)vÀ<{Ð?…¦°%?oÎò"¢æe?d¶¹P¸ÅT?–×I§Ü)<?"2æXó ?ïÕ>?dg?eȐÔJ?@ôRw¬Tê?1Œ£³§K?sBq'XBg?e&sH&$4FGL J1059.2-1134?ï1ϚÔÏr@EWçl‹C–À8*obŽj'À;ˆÅFƍî@0¿¿s@´ó\ƒŽ•?–Ä|=µ'?§*ò®~@
 "S.{>@#ùñÉ¿ÅžÚK:ö¿àˆbÚÀ«V¿âd["{L§¿á!Ä«–`¿å°pÀÝU[¿å7i=±;wAGNbll3FGL J1059.2-1133PKS B1056-113?ïÄØD*Ù*?_ëˆ5S?1yPlö#ä?JêÁ0ºo%?||HãÄ`?œ&Ïön?ï"ªÀ]í?¦¨'öBþ?^aªo<³?r¯Ò\>‰?™Â±Ù·î[?¦7êºÿÙñ?ï5ÈòUŽp?†giD?qZbÜ­Úã?n+æðü¸ï?"ðHþ"»e?ƒÂëÞcËQ?ïÉJ¯$Ÿ/?f³·+UŚ?UîXÏ?I3"	?uö¤rdØ?dœ÷~i‹4FGL J1059.5+2057?녗¨N@Oâ»ìª¸¦À:"'Gm|ÛÀ<o¼Õ±@‡Ñðøü@-›ymª(?Â;Ñ&ù"?®h˜Å´)¾?äsmµæz@	œ²êx"K¿ßÏÙ\'HC¿åF,iëV%¿å´üÌnÙ¿ä'zޢ߿ï\tÜJï?æusê³g¡AGNfsrq3FGL J1059.9+2056MG2 J105938+2057?ï"ç6dö?°‹ö,qJ?m:TžÒU?}r³Gü?˜˜…Y ‡?®sؔ?ïŒ@èÅNð?Šð*x,+B?J+i''Ùz?Y›wó±ãk?‹M5"p?‰–'{¬aJ?îéw‹»Žå?‡@Xýú6?uû¾¾ö<?n|šûŒOª?RØТÓ?ƒ‡ÐBN]?ï"F‹§&?sJ+Kf?izЫL'?Z[MÒ>a?"ϨñC¬?p`óù¼~4FGL J1100.3+4020?ïàØˑA@OÈ<hfÀ:7|ˆçš®À<i÷_GŽ@ géAørî?û…tH§8¿?¾ÏtòÆ0¦?¼ìæÞýÝ@øSÜ &ç@I¾ð–*¤?ïsy³J¿âëÈæà>½à ¿(¿ÕJí#¯\¤¿ÙXI"ç«¿å#傦8AGNbll3FGL J1100.5+4020RX J1100.3+4019?ï¶
™L™?w'¹Ÿ/o?V¯Òiv!<?Sq—AZ?D†ü+\?tßò£s?ï#c±Ô$ï?–ß\î­È?f
O¾¯ÕT?o"œú;~?˜ÑßÍ¥gW?"óŒFàôÝ?íÑzÐzŒÓ?"äãŠE?}JìoÁ^Ä?joÈKÄOV?¯>õj_ñ?' &Êr¿°?ìhÖu"¡ë?™^ظ×û?™N.Oùr?"·RæÉ??¶eÀ¿šòK?–
¶óÆ'T4FGL J1101.3+7017¿íñÖØ¥"E@Fÿ¼ä!À:CÃz=³ÀÀ:ìL>œóÁ@ÁÿiW@6
éh?·©׉>¿»iˆúe@G£áñø@]˜oVпÓÈ^˽X¿èéQgÑ q¿è]Áa^¿©¿é"'Ž¿á;Tiä ¿â\‹áõþÊAGNbcuGB6 J1102+7019?îzÜöÅ
?­i4ÖlàÉ?ƒËQ.l©?"­,Ó$?£œ¯\H?«*þ½Ó!?ì<™NMìã?ÂLQ ÜX?¤—½	Ý?ºÎãgd?³Ï³¯
"ø?²1€PE?è•ÒQR?°$|¡$Rþ?¤UáˆåX©?–4^V*c?ÊâF}d‰?­'%Gí?Ðb¯¥‰ã?»¦2¯zi?{'2íª™|?|Jýˆ³B¦?ç˜YǘåÛ?»É_öɔ4FGL J1101.4+4108¿×"ð§`ö@O¹É>¢ÒþÀ:{V'Ý¶À<~CyÒSõ@ ·~"Z•x?ú#¶¾mŽ?ÂÅ Æt+?ÁȚx'·"@´ªFJ@‡¶HüÉ¿ð?ïÿþˆ0»Š¿Õ'îdw"÷¿Öh…ºêw-¿áÇq^-O¿ÌɄƒ\ì?AGNbll3FGL J1101.5+4106RX J1101.3+4108?ïÏpùøÆ?sËјY‹é?M4G7ÇÎ?DÂDòxŒ?t ú¤m?sOÙëyþ?ïpJ«Á?ŽÍO~ÙM?Uý— Œ?aÀÀêsp?œ]E
ä?Œ¼Jvó·#?î|áß"û?Š
…rše7?rÑϲhÆá?g,(ð©â?¥×¬û¹§y?‡Þç'‡?î‡F%ú#?Œ6BÂ1f?‰3ðŠ¡Ž?r¯Œ?àâ?©g>¡}µ€?‰FH~^=¬4FGL J1101.5+3904¿èWñWŠoI@P
j½ãû½À:ÊbhÀ;ÛHHn-Û@å	Yšü@·Káâ8?½š)¡äì©¿£âX¥2©ö?ä¤d~.Ú@¹ññIƒØ?ïþ;â¿ë-i$†È¿çWöÌz—v¿åé<oŽ¿ïþ%–c.¿âïÃÙßAGNbcuCRATES J110130+390434?ï"(ð•>0?ˆ\ïtÀ¼?'&åbsĂ?'ÿdäIIá?r¼ðy_°?vIfø¾?î¢EíR'?¢k5°`&z?xA
ž¿?ƒ^Î8÷XÆ?¢Û£×—? çsEÝ?ê´ÙšD²	?¨ž—}˜G?§‡0ü¶×€?šwmjú†S?¾•š¯ù?¡…6$/Ós?ì»ÄÙrfW?'â˜2¦&?¡ç¯Ç梁?"Ø*œ?±.Py{ü?•žÆ_È]4FGL J1102.0-6054?áYz)^?ž¿éæúàÜNJÀ7äè¼í[¹À:!_Ìqç@ñèÒ@Èÿ΁Ù?¶Hê¿üÚ²?Ñ XšËÈÁ@)Á¡ŸØ?ø_Y	¸&?écáPè¿Å§¼Ýk€'¿æ|fÃÊÆ¿ê"eҐ[¿êZ³R¨D¿ÕcŠAGNbcu3FGL J1101.9-60532MASS J11015838-6056516?€7¦8èx?~à87?¨U?è_'*þö¿?ɤײÀS?Í~@ðuœ.?Énœ¨¾÷í?€WúX1'ï?ŒÍÊ^û`¦?å"Êf¾1?Ç	ŏn,?ÔU¬pú_?ÆÆ6S<ä?¢ÙFŠ[ñô?B׸¬è?×]µ0"?·ìÂãD–?ãH<¼Ò(—?·Ð…T£©4?JBÔ¼ûí?9'à"þâ´?â6Ïk·"?²°mhc?ۅ@"']|?²§N5]4FGL J1102.1+2249¿ïø»ºD£¸@P;$_ZÙjÀ:Ö0ã͚RÀ<y,;È-+@øãýëÓ£@
…É=?Ñ:~¯"®?Ïg	y{l?ýæª|¦D@B9_E0¿•CÐå5Nk¿åg©\…<¿ç›Ò>%Õ}¿ï=ò@¿ïՀ/eHY¿Ó0æ"ÀAGNfsrqCLASS J1102+2241?îâ.ˆEs¿?«VÅ|즢?tƒ,EZØ?u[=")kG?ž™cåúÑú?ª±p¨r?ërÛ-}Ms?»ëÊw v›?¨MŽµ?¯"ëNV߄?¸ZN?³Q®ÔM‹»?ë!ÐVr?¢ïĶåè?¥P€ZH1?'–˜Ýì8‰?¼+Y=K[?FÚU'Iý?ê~všd?¤†œó¢>7?®7‹óM"?š«l8š[¨?»øFQˆÚÉ? ›zo¢*4FGL J1102.6+5251¿îâˉ"J@L¦&€IRÀ:҈
%ðÀ<ʵ1¥"@V7éPf@¹eç»?˜ùJ"2ª?Ë*Pv%ã?úI·¿Ža@xh??ߺé
55¿âÿ^šj¿ê˜±¨ó¿æ>mhc¿ïÿØȃ'ð¿éd}Ãz=´AGNfsrq3FGL J1103.3+5239GB6 J1102+5249?î÷""ím?»¢ÅòAˆr?‰Ç!Ù~~é?§ÿ­}+·ë?"8•œòñ?±T<¹ó=ë?ïyc¼œÚÃ?Œš(Ï|N?Rcºýì؏?båïG0ÿ?Z™y´›?‰ýèÞ÷ù?î1"O#s?' xJ#?‡H·pì±?y½ÅaB¡?§¨NÒÃù?Žµ¾˜âÙæ?ïÎó
–á?`àÐ* æ?`
š`ºÊ?J\Õ˜\?p,­±Ä?[ûÑô²4FGL J1102.8-0148?Û~4R0é@I~þ£ßm¹À;¼pñÚ£OÀ<ÏQÕQ×@#E@tI	?÷c¬bäÒ?×(§¾öJu?Ì<ì™.:?õâíÖ1Ð]@J}ғ¶¿ïÿ^à54j¿ï'7*8¸®?ïøÞ6A?ÌõýR.Ì¿Ðó~}ÖÅ¿ã8ì£^iAGNbcuRX J1102.8-0148?ïŽ`ØýÌ?…×ÎïuÁ?Išjf.ÕÆ?CÇi¬…û?ŠÎ#*î?…(9¸í?ï5ôßc?¢f#["ä3?Uû΋6Øò?p¼C|c??—á¿ÓÐ¥ê?¡åFšŒDU?íAœfïV?™Îã684;?z.ÿ«t´ê?møhnϝf?´P,ÍÎé?˜ÐÊÀ	·?îuíœ?™¤¯ñŸÍF?O2Ó#N¨?M|²ŸFPi?®‹$lÿ?™€ÒáÌm4FGL J1102.9-5628?ètÐ*¿
0@
J¡¼}Ê0À:p.Ï÷#¸À<¨(÷@ »a•qA@:ëÄØí?Ç8§?¸Ÿ.ê#?íè*Át©ö?ÿ?®3Yž­?ïÿ!Í°"¿ìTç4¿³[H¿Ñ*™¿á‹	³Ýè~¿á%&_楿æÔù è­ÔAGNbcuAT20G J110315-562635?Þº:'åؤ?ÂF÷©"?u_9±ª
ú?lbH#vö.?àx$K)¿˜?‡pmÈÆ?ßF…yr†?Ç_¿Vžt?ìã¢j?ŠY29Uæ›?àA¸3T?ÇDZ
4–?æÎ6#=P?§Ñwöâ?•³yÚ1ãŸ?|iº} h?Ñ\âÛ&?¦‹Ö$ð`?ç"Kwžu?£´ÍÏ6¥?'æ"m30!?}˜
êù'Ý?Ïv@{ (?£¢5VFã4FGL J1102.9+3014¿ÝõÓ4<j@P"
ú/§À:¢.›
³À<"îNý"@YÚ;JXê@!ï#8ê,?Äܸ¨'¦ã?ÀÖYh|?óQ+¡nz1@o%ý•—¿ÑW6]48—¿ê€O ý7¿é$¦©L•¿ìYƒßž
¿ï̚!ÿ¯"?âÉËûìu	AGNfsrqB2 1100+30B?ï6Ƒ0ô:?š_}±!½Ñ?fyß¡i?'ÖÙ.®˜?',À®Ž?'ÐpÚ?íE]·ó€d?´D¹_¯?"¹-šh?Ÿ˜â¾
&?°¦ÆÙÞ9E?¯?ñ†áŒ¦?í\8ˆ»kZ?"ý1{Pg?ŽE§ÇµÑ?~Z99‰h?±Uˆ+®q?'¨ؑ%»?î4KË¢5?–k >è
=?Këܒ€Ž?µ$¹¸k?œ0ª©ù8Ã?‡"âME…4FGL J1103.0+1157?îtÀ	¬t@N6#=òªÀ8ø€'Š×_À<uƒ9ÛÄ@ÌwȹlÉ@aGãÄ`?©6æ'xÀ?¸ÿXÿåAÒ@
@-¹€@çÀI‡¿Ø9ã{î¿á¾«6z'¿æt~¢Gh¿æfOõá™
¿ë aÉÁ¿Ý™åóíAGNfsrq3FGL J1103.1+1155TXS 1100+122?ï¼.Ñ5M?€Ù·5AG?Q¾1ѧa?K§Ãƒ¾úú?}†aŠðït?áÙA®w?ï"ù¦hŽF?ˆo…È°›ÿ?J óy?Y7¸™L;?‰W‡4D^?‡œ¬\â?î™ËiߦÆ?"7L£¿?™˜
?i?w»T%§?¡üã^µÎ?'SíZýϺ?ïúZ³‰b?8¬f'µ÷?#YúœUeØ?È(ˆ`–?BøŠÅþ?6Wx`Šþ4FGL J1103.6-2329¿ïÀ¶Íö²=@@‰ß¹8›RÀ9ï(ÝnۀÀ<![Ao6@ ø/']5?üNÞõÄ<Û?µ/Gì'Ü¿a*8'æÔ?«àÌVn@Y­í¹?íÕ»=®6_¿áâû{8†¿ãÌ?Ü¿Çïϛ´&
¿áÓìCÇ«?c…—ÓPAGNbll3FGL J1103.5-23291ES 1101-232?ï§1R?}ªõëaþV?Lxߍñî™?Cè²&,?"vn'TŒŒ?|CÒ`NTï?ïoÈ¥¹ý?è¥CU?PÜw—¡?^ø`]ØÿK?ù*löÖ?‹ûEÕ=?íX])";?—Ø<º˜£?ûã¥øȔ?qúON9r?²ýš?4E?•ÖÂH2­¬?ìxèVç|¥?™šÌ4º¤a?…¨¤v?p¾¤!‡»?¹–9"¯Œ?˜oš
Åã4FGL J1103.9-5357¿œhüŸ¡'"@š½†ìÀ83á
Ìq]À;Tª:э&@‰K+L‰ñ@-ÑyÚ·q?¢ß#í"¶?»p´yß@kK¯Ri@2("ž¿Ù"iʀA¿Õyœ^E¿ájè¬&d¿ám¬@eJÝ¿æœÜ¤Zé¿ê*ȀŒØ@AGNbll3FGL J1103.9-5357PKS 1101-536?ï=QaÄ+?‹¢|(@©?KI|!pÅ?Bñ·øù9¨?œ	óžnö?‹k%¾!ç?âQY?®ãqµxø?T¥pU ƒ?u,í:m£?¤a6ZÀAd?®¼øö=<?íºd`ÕMÍ?œp
µ§Å–?'àbrŽå?‡'ï×AÇÓ?«iˆ¹dÐ?˜%$«.¯?ï˜E|)ÊP?sbht~a?JŽWIêÒ??
Í+®:'?ˆE»€îÉÕ?rÊ[€Ì4FGL J1104.0+2611¿»B®æ²Ñú@PØ¾r–öÀ;-C8dÀ<Ì]°µ?@ ԁ÷çX?ý?óÖ&ã?Ò+ݾâ~e?Á,á	š³u?ïUa%´Åo@Æ̝|þ¿ä9&A³¿ïæ,Ÿ›;Z?ì°Âtºg¿Ñ´îV,\¿ì^ܙÉjB?É/-5A*AGNbcuSDSS J110357.29+261119.1?팉ù?®¶]IÖc ?msûi'o¶?eBÄA¬Ú?°ÿûÔë,+?®A?¹P¶
?îù³èÐQ?Ÿûþ*ÿ{‹?gŒ®x^?yÁ©óҒ?×íôlA?H²ÅJ­?íŽI™í?š5iŠO¤?‰h­½Èó?|­»ã»?³Öa[w'?˜+ì«÷c›?îÇeO—žÊ?âMÕsV$?pmÏfKŸ?l.
ّ[?¡{ñ´	ß?Œ-!̈́‰4FGL J1104.0+0020¿ïÈÛµ ®@JiÝS¨À:ÕÀOæÈÀ<CHɝm@³k;p|@X¥}Ójv?Çg}'Hs¿'Âþ†r?Êd|ZÞs@Ga¶Scª¿ç¥ Jù"–¿æš¡¬bŸ¿à:â‰Ís¼¿îc!ãT¤?Æ8'}sHL¿ïÒìk΅4AGNbllNVSS J110356+002238?ï'™k}?~—
™z}?[Ìùqãô?d48žà?ˆ:h¿˜?ŽbÁ«BâÛ?îîöóæ¯?¡9©Õ½ì?]abDõnÀ?j"˜]¦»ö? 4…~™éª? dìfÁfú?í¤ß7+?—°|jqVô?‹×ÚF­ÿ¦?~ü7i/¹?³Çä 0†«?"acžùˆ?îôØg°ú?6UÄ¥ÌÖ?IùŽÁ?J	 ®Ú? J"N!ëÑ?ŒðMP·Ä4FGL J1104.4+0730?èî4Tà÷@Lùfb4¨~À9ÎÕxlù(À<RæP+'~@ת«dÈ,@ϋÃîú?±ˆŒÖ脎¿ŠÚ6ÓâÑØ?Ø.‹-Æè@ñÑØzU?J´·,Q—¢¿æT²^âc¿æWúȈšn¿àzó†tù§¿ã{Ö[åÚ¿è-ç>"
¹AGNbll3FGL J1104.3+0730MG1 J110424+0730?ïºã¨ÒÒ?y½ïSž¡?O!'# -î?BµÝk?{?]ç2'º?x ZU‰#å?了s5?ƒáD%yéû?C/Áwlä`?U¥ÛeV4R?…_ĬdØ?'³¿¬{W
?ïEÜÆt®?yõy[&?G?eñw¹•TJ?P8¯hÎ?"†8:7ƒ|?wö-±ZÏÓ?ïÓ»ÌԁT?]"Hêš?XÀȓ‰N?DÏe×=¡«?p©cšsq?X¹ë¸ï4FGL J1104.4+3812¿ç%ÅЕjq@PBIёXÀ5•v¡G
À:Óyq@'=ŒþU±?ûÄ£ÿYè?z}xf»?"×BÇzÓ[@º'®š²ž@Ô9ùËÞe¿Å¦²Ü¶¤Â¿Õ$è[Ÿ¹¿Ü‹Ù?Áa¿Ö¼/ʱ•¿ÞÙTšŒ¿ÓH__Œ«AGNBLL3FGL J1104.4+3812Mkn 421?å¯ß[»>Î?ÈpØ1Ì>}?N\uRƯ?\ê
@j?ԑ:ÎØþ?ÈqÃd!ª?ïEÁÿñ†²?œhuÿòÑ?e+A2îD2?~—ÍÈj·?"¢WÛqa0?™'ê2+í?æc‰-¦x&?²Æ!sLöH?'·³=Í?ôZHü*ý?Ò
rkß2å?²£íXd–?ïÙüê £?rh=¦éh?ÿ—"OÁ?"Šv{|´?r"'ñOîH?rZbX孞4FGL J1104.9+5748¿è#ÉlßÁ
@K	pŸM8À;cpè hÀ<¿Pû›@Þs1s•@ÈPïܜ?ÃNwëC?NVq¬˜@	æ4á‰t¿í⯢št5?ïÚ==£#±¿í²•~æ¿Ò•!û'~¿ãÎCYñãÞ¿ïÿûÎBÓAGNbcu7C 1101+5808?ïû"Xæ?PÏG¬lI?*¸¯T??6rî¡ Cþ?6á%à³?Iט€×'n?ï«Ji'"F?…y†¡"»?CmÊ>é´¡?RÝâm•˜?ƒöˆ÷pSl?ƒÛ©¨ö¼¶?î{è|nj?•áãÙ á?xôOÕ9¢?wß´š¨¿?¥/÷}' ?•I+él*?ïæ%ǚà?WNêÕÛ8­?RÐ¥ƒœ:?J~Ióú?`y‡«£Q?P0oʜ&4FGL J1105.8+3944?î¨Cïª-¢@P0O"}ŠÀ;/øìÀ<"Ž7£@N´¾c(@מà*w£?««u+%¿¶ï«^"[?ôÏ|ªuŠ@ƒ+ÍcJ¨?ïöaD=¿æ6M½øô¿è;$,/3¿ãÓø:8àò¿Á')™¿ç¥0 Y;ÛAGNbllGB6 J1105+3946?ïwŒè
œm?™rX@Þv?a…Þ~"x?[‰½tX?»N]´ÿž?™)úF¶sÿ?ïPIñU?"áwè7,?[&)hù£?nçWÒ¾Ò?"D_>Ý¿X?'Pö6Ë-?íätïY?"²"F¸?v‰?gýVð?g™Ëœ@ðh?®îÄφ?"{zö©?î–s̄
…?'÷ÈK0|•?saÙÔî6Ö?o±FeN ?¤,‡ý!ï?Æ[y
«-4FGL J1105.8-0731?ÚB6LS{ä@Gx ě¥ãÀ:ž'jöîßÀ<yÿ ^°@™½€Ô@ˆR]S?¿óâæ>¸Í?qbÿ»Ô°?³|{P®CJ?þ!/}F&Ö?ï¦rÅð9¹¿ä†ÿ=T<¿äûà^d¿Ù¦-¼%à¿áE}Ð:k¿èppçɨAGNbcuNVSS J110547-073235?ï38aˆh? ÁNKûb‰?fƒd§e"?\!ä•?–È'âjæn? 'S­÷¯ë?ï8FéÈ'?']+‰õÏ"?XH"hû'O?bÄCþ¾?—xTü7B?<²P3ú‡?íëdäšX?çôTäx?€—·Q¿?e¬Œ­`j?­Msëȅù?Ž'6ç}»|?íìãà²Ì?‰ùì'.?ÍÏ×Å‹?uŽ@
™'Ÿ?¨Êæ–P?†w¤¨¥¹4FGL J1106.0+2813¿ïÂ}ØÆ@P«hœ¡‹ÖÀ9TWuÇ,À<NÄ3¡<@ýñò¡Æ@®iŸÖÊ}?«ï°GÀç?²‰»ÀŠõ@¤m'ºZ@f,I	3Z?äQXí×ßP¿â	û+"é¿å±€`b–M¿åâ£cF÷5¿èۅ⭉¼¿æðÎ3Õ¢AGNfsrq3FGL J1105.9+2814MG2 J110606+2812?¶,g"?†sMŸ¦H?Q\¾B»Ÿ?Gï{?ð?…èú×?…"^s?ïˆÿÔ°î?Š*lWÖËñ?MϪ´u?`Ç_pâx€?‹ã¹Whë?ˆoËÐØ:}?ïœ}Ìh"?†|`eJ'?qOzz0x?cÍ?+uT?šØ'§æÝØ?"gYÿ¹?ïÂ.WÇÅô?h²¶´Êñt?iÿ¿Ág-?Y³WëHN'?r!Ô<<RL?aœ\¼4FGL J1106.2-1048¿¤á¤+9@F$ÐgŒTÀ:÷!' ÿTÀ<U1Š¼‡@ôðVÝØ@Cœzª?Â\x¦Ú'¿–¬fzÞB–?Ò»-½þR×@¦`s^™¿ïÒ͖ h?êÜøɪÙ]¿âyJ]d¿ç#•Þùö¿Ô±JG
¿æk¿Á¡u†AGNbcuPMN J1106-1048?ï)þë8e?–Eh2f`?e€´a¯§L?_¿Jô=¿?˜þg?•€"O'?qAC3?ŠZy`«Œ‰?BgS$Çu?N$?㉃®?¯²*|ç!?‰'ƒÝÿ¶Ý?íÃì[]s?'èÍ<À	à?ƒ`ƒ5€?qvb}þS?®é2i[ˆ\?dÕtKvû?îåxõè@[?ƒÇ
·ï?rCZ'!r?dÜ©âÈ`Í?žÀ
¢W¬T?ƒ†¦<4FGL J1106.5-3646¿âEn¼§@5€"xÐÌ6À9ÉÌIN†À<D¨£!ؘ@IV
M·@ƒŽ)ùΎ?´}íì'Ô?³íóŽ¶@VÆž@
ï6ŽÝS?ïÿÐß´¿Þg=;tË.¿äø~+	Ë¿ÒÞc£",¿êJÔø³¿Ô¬Âû<ÍAGNbll3FGL J1106.4-3643PMN J1106-3647?ïµ£êëö?xj|t'Ë
?TŒ…n«?MóPeè?€tÛä•$?v½
{¦Î¨?ïx¶Õo@Ð?äiXâá ?[®/Ë7Æw?q3WY÷&?Ž\"ªÈÓ,?‹Z%FÐÂ?îį­× :?ŒÓ_ƒ°üÐ?|zbÄH]–?wÓT/䥥? %¸Êð°?‡ê±ÒˆT?ît¥-ƒ	?"µ:üy?‹­"6g<?sbþvÿ#? PêZ5£?\ÂSB4FGL J1107.0-4449?‰˜7ÍTe@,hÆ÷ µîÀ9!—q¡-À;ã¬ÍSŠ@kêÈ5cd@lŒPû?²
	È««?Ñnîàå@¦ýòÆ@D€t¯_¿ÌN
$=H¿ã•è41_ô¿éÙ(?º*3¿ë"` SÈ¿ëÂbæ%z¿ïÿ£NNA¬AGNfsrq3FGL J1107.4-4447PKS 1104-445?í\uT'Û³?¬úùÆNý?²aÜ-lLÒ?¬Q¼šÿ2?…ÓÉo欪?'c…¥JÀ?î]0/)¦?¯Y€aø$?‡ëUóT€?™Ñ$ÊÞ­¢?¤2'ž?©fÎcó¡?èË)S@Ëi?¯ye úÉ?À²²G¾a¢?§Âö/~á?¸APÖ|áx?¢X¢@ö¤?î‡Ö¥çà³?Š‡ƒ×?"ÿoù.³ç?€/UØǤ?›»IÕ5§?œâtž24FGL J1107.6+0222¿Þ? î'\@KvX£/D'À9ÙÒø_øŽÀ<?x½€ÿo@¹Ggž@À¥ýU*Õ?´ÀÿÚÁ,¿Œ:Úzm?ØuzÖµ?ü]JÑ_ƒž?ï••9¹¿â$çî'C¿ä90m†X¿ÚÃ*¢8¿ÚA	8x¿ç0ãݵ}PAGNbll3FGL J1107.5+0223NVSS J110735+022225?îp§ß×?5ÐpÕ¨Ú?yšü1«è?j^Ð 
N¥?«Å¡Âˆm?›²2/Vì?î·î­B=z? å€ùeE?r7vÔÿד?}ì2/íúª?¢:&Q<-n?âry»¸ª?ìõ•\‰FŽ?™¸3–­h?Ší`tˆ?x¼ê-7?´õ©'J?—S»+}?ëŒêÛ@ä5?ŸGbÃ`ô?¥áQ=Ž_?¢f9»?¸¨‡1®?™©5§x4FGL J1107.7-3042?².ØãÀ@;R¤ À:Õó‡K¹<À<u¿î¼@v™!N¯;@éœzõj?Âð¼@7¨Ž?e1Àz*©Ò?Ÿ˜<æÿí¥@»^ÃYÜj¿ÛMšÝ¼^@¿ÝǟÑÁÿ¿æ}‡ ¿ìTÃ;S"%?Μ­ 6Á³¿ïÿÉy[5±AGNfsrqPKS 1105-304?¸ø¿©?†c;à+>n?\òð7r?Y&a·Ð?…{³Ámî˜?…Qù½PqÓ?ïùU'¥&?Š˜`'ß'ã?Drå~« ¤?Wió{€µE?‹:|^,ã?‰A·™Bï?íÂê?ÕÇ?'ÿ¬,Ý?"šTÞø~?wt†žc¿?®ªÆÊð"?Ž ¢çIŸ³?ï¯ú
M—t?rËÖ=qd?8ñƒv`6?:?QªÜüÒ?ƒ9ñPé8:?r¯†_#±²4FGL J1107.8+1501¿Ò_¬wd@O‡EŒÒ
úÀ9À]''N#À<<Ò@ª;@+ÍcJ¨?ýÄÔ`?ù?¶šCžÌo–?µÀf#z@By<,9@0™)^"?ïÆ-vZÐ0¿àÿø¾m8"¿Ýw¥Þ¡`¿Õ7Í¡³ï[¿áp #‹öC¿åšíV°AGNbll3FGL J1107.8+1502RX J1107.7+1502?îäœD–?fAþŸ?sð|BX™?dtÖҏt'?žp^Fõ—?Že
Ô>ªµ?î{$ê÷µÖ? ¡X[–G«?€7'Þ#y?‡€ëOxȨ?¤?Í,
Ù?œjùc""r?í'}K¥D?šÖã)hω?‹j—˜­À?{ZzÚ·²;?´	q4¯À'?—nŽk¯B¶?ê1…qwj?žhjš!I½?°¡>æ[w?'ܤ4}_?¾4îaé<?˜fëݧ£Y4FGL J1108.7-1844?·êçhûQ@BçÁß3ÞÀ:Ò
(ÝnÛÀ<kDTæ³@¾òÖ§l?ÿž\\!i?ÎÏÅåýËG?ÂU½ ÝE@?ò®²Jj‡]@Z©è"8?Ò ~:Bœ¿ãOäÿÉy[¿â˜¶DË¿ç¡â"o¿Áô×ÃJíå¿éø@~AGNbcuNVSS J110845-184505?ëb‰Émè?±™xKE?€é*ñ"ì?uØ5½´(&?ÁgF+9Ž"?±6â+ö?îÍä:q!?›ÉŽ"Ñ)?hmÌÕ³‹å?qï6ì7Tï?¡šß‹"¥?™)ÄLS
"?í•»°¥?š)áµ?ì™O}?q‰Ö¢Î?µ
ÑÏW-‰?˜(1j)?ìrbä/ÃH?™Ú…Ú; q?t¬9ӚŒF?mO4š–Ÿ?»"%AH<þ?™ÏsF».^4FGL J1109.3+2411?äø±ÆÐÎ(@P¶'Ìö¾8À:?9ÉOiËÀ<g¨"1 Œ@ 
¸÷'Øã?ýwM©Öþ?¼çýÀ4¸ï?¥uø)Çύ?닫à.@[¨ý?ëÄ'¬í3u¿Û懞olI¿àÔN¡MÿÖח`Ú5k¿áüÄʟ̿̂ XÐ{®AGNbll3FGL J1109.4+24111ES 1106+244?ïxš:ÎýÀ?úfÞ-?dì4‹}?VRº"b\J?Œžm??,¬?|Ìæë[?ï]gû—Ú?'ÏöÖ/"?Xîº'íÞ?cšúõÞq"?'Ä?Tê…ô?3˜O¨?íÐâê>ê?'Ø_'ÆΞ?€InŸ¶¨?k°h»ÿ?®ß")"ã¨?÷DOßk+?í»Â(èÛM?ŽT²O©[?­uS¦4?uÄBU`ëG?«í¶Èx&?Šsöü/"4FGL J1109.6+3735¿ÅVIZ3t™@PŒ°á´»^À:¶'néšÀ<…ý	«zm@ óÿ'¥?ù,Ø:¿¯?ÐKs›Ù?ÈTµyt
>?ø7ó÷´$@	àŸµg€m¿â¢X_g™—¿ì곝PÞ?¿ÑO7
XH–¿ÓØLÝ©=ü¿ßŒDý
,T¿àcŠØûAGNbll3FGL J1109.6+3734NVSS J110938+373609?ï6Ñu/?§áÖÓâ•'?kH22h}n?¤c}ªô|'?•Óÿ‹

S?˜üd¸]n(?ïœû1ü?†Ñ%s,Ïÿ?C*8R±Zl?P…¢51"?‡Æ]®UçJ?†
i<l?î62'¨2â?'ÍátFB?l6©p~õ?_¾Jà—é«?ªÙl>téÙ?'Bd·ï?î­¢1­ï³?‡_KŒ_xT?UXèþ0¯…?FynQ8j_?¤{/P?‡>mÕj}e4FGL J1109.7-4814¿ïÓ¿Q±oñ@&êþæûLÀ:³þËLš
À<ËRyI˜@øS*I¦@|š»É.?Êh'äÄeJ?Á	pT§?óøÜP'`@í}ÃOJ–¿çÕ\¾Fø¿àPVXÍ÷¿ëbâ¸Ç\K¿Ý©àc­y¿åzэ%íпïÿÊPʇAGNbcu3FGL J1109.4-4815PMN J1109-4815?ïlk¬Ø?'–›"k¹?``^V¨?_Iž—ZB?f~š)j?'ɦi<?î"Q¦ƒÒ.?¬('Õó?aDÒ._O?syîÌkÔ?¥¦˜tÜìJ?«B/	ÏDÊ?í}|Z¼c?™øô®~Ê:?¨ÒµiŸþ?rÓsyU_ó?²þÆI{?˜Óûm–¨?í·'ðÒ:×?",ÿQi¹†?o£öÌkÀŒ?\òsl¶Ã?±I Ã
ËC?'Âäuï4FGL J1110.2+7135¿½¹^+À‰Y@E°U2a|À:m«|ðìÀ<­ú4ää@ ÛN?üºØÿ
6»?ºŸJžê	?ÀÄø(e¥@Ÿãåî@æÏ¥DG®¿îfºI<‰ô?ïœàÁ q:¿È¶ÅúJ´Y¿ÚI›)'Ÿ¿ç*J+Ú¿¿=ç—({AGNbll3FGL J1110.0+7134RX J1110.5+7133?ïÏcÑ{Íä?hÉ°ƒ$Jò?]JÞÚä?YlL¹qğ?pûoâ!Vú?b)t¨ô&?ï/u.hŠq?˜üœ?¥IG?hšÁúÿlŸ?xRî?$tª?–þóŽÄP?•"arœó`?în­Äš?‰Ýî–ûL?y@/+­'g?iò;½üƒ<?¥íÐèê?†ÜhG2i?îMóÙÔgC?‰0uC]'?˜çð¼À¼O?€Øýþ }¸?Y"²[Y?€<'×?4FGL J1110.5-1836¿Òp B¯kØ@CÜ­¡À9ñb‹"À<0îP«?@ .l6˙?üo"èbT‰?À7¡?Æ!w±<y@ûB±Á¯@š#SAE›?êéTWp)^?äšs´,Â׿à´uBwHâ¿Ú{Ϥmˆ¿ÞìTQì¿çGpÂ_ágAGNbll3FGL J1110.4-1835CRATES J111027.78-183552.6?ïË_	'
?nȬ±Ùl†?bØ{Þñ%?Xªª¬O«¬?pä=H{Ö?h)Jæ&<Ù?ï…8¬ðò?ˆÛêœ_×?RX¸eÌÌe?_ÁY@û@¥?Œf½·	à9?†¶ÑXŠµ?îÛ(÷^Ô¢?ˆûk5GÒð?u¡q3>?l¥hÎÙW?Ÿ2"Θœ7?…a*ÔÔ?î«4¨$?Ž§Ñu¦lº?‰K9ýk3?t©÷ܫϜ?©"~6$Ñ?‹>ƒÐ—ì4FGL J1111.0+3542¿êÌc#'z@PÁ)^ž	À;Qχ'0À<ݐ8ÇǪ@ BÞ£Žåá?õ?\l¡?Ý8LA÷ò?ïñð"<jê@ϵdÑ:ñ@Æ¡Íš¨?ï¦Vv.Z†¿í³Ç™kv¿Ê¨# 8Ü¿ÀœaJÙ«¿èÁUj• ¿ìcõrÞCîAGNbllFBQS J111056.8+353907?ëKòRމæ?ÀLSvª>?¥Aá(6aÕ?¦p""G‰?ºÿ|ÔðÞ?¼®ÈÉ¨?秜ÿÂ1:?ÈMH¶v:…?ÁKým†ö?Ãÿâh×1Þ?ÀŽ"pDü?¶ÒÿoçÕ?ëֆ¬DÉ?£xkš??˜X)¥[?‡1|žúÖ\?»J´"u¿Õ?¡¨é†LŽÙ?â×RD[Gx?»ÏwM†}?ÀZIÃ	<ô?·}YCäs?Ò$6•Äҕ?¹1~±"›4FGL J1111.4-4624¿íóÁ»;Ø@*œÜD9À: Ô`?ùÀ<-±2ã@gò'"ï@Zp?Ñ_H$†òù?ѵ"2E?ýü+_)[C?þû0ˆ!¸?ã¶i´Ï€¿çàæ_E	õ¿é–'q¬ë†¿â¡¬­O"¿îÁ
F9 5¿ï6¹ÐpÆ<AGNbcuWISE J111127.39-462504.0?áJb* 
®?Ä@‡à[øV?ºÙm® w'?´ÏÍ؆8ö?Ö´à@7Ì¿?ÃìÏê6bÞ?æ!{ìÓê?É5è䫚?µ•Ú¥e•?ºb}s=Í?̯#@ý?Äû§ST}µ?æµñÓÞ6?«v˜iŽá?·.òv
?*i§óá?ɔ*ý¢ú%?£Þ!¤Ð¹?ãè
ùîI?§ôöB¼?µXÄ|8Ô?˜N~Z"Ú?ԃþâ-:?§Á$ÿ©ú@4FGL J1111.5+3455¿Î
J¶‡'@PÒ¼j~ùÛÀ;pZÇ̲ÌÀ<¡`†R"ø@"Ç~Õs•?ûr
—~?ÉüšoØ¿[÷7	B?{yïÃê@€(R¯zW?ÖIë;LÝ(¿ïþåþ÷í7?ïÿüÚ±'Þ¿Öøè^£¤_¿Ýî2BrkW¿å»l°Ú(AGNbllRX J1111.5+3452?? '? ÍÑ(=‰?aáµd}h?Ÿ_?U¿Ø?"æBÞüüf?""ªÃjX?îÎòKA
?¯³Åßð°?b¹êö§šX?sãù`S7°?¡å<œƒµ¾?®û–{ãŒ?ínš'H?—¢HŽ‰àè?q.óÎ\÷?[þ ßï°?³xNWïö?—|@]ƒ?ëNˆgB+,?©Ÿ=¸"1?v
¥b»èÐ?s¸iéP?Âq7át
?©—T"€|4FGL J1111.8+4858?ì`~h÷Ìf@Nu>ÄaÀ;׳¾
ëÀ=µš &@!Yy²s…3?ð4Âkñ?çÒÕZ::?ßê^bá̎?ôéËº~@ò00õ@^?ïø÷Bl64¿â~p·'©¿ïÃC·õf?îVų-¿Óm'©èò¿æjmAKúªAGNbcuSDSS J111158.89+485701.4?ïQ·Ö;ÆW?¡»;X»á?dˆþ!ÙÔ?qpwLŸÍ?"9ÂùÐ? 	VÎÆ2?ï«ñ0{?‹†£w|°?Cª+rÓ8æ?háó(N7›?ƒÉCMí•?ˆ°F•Ì€?ì¡2ü?¾?¢ ¿k<õº?"þÙ4?]?€5>lY?¸d¨Bàâ?¡yDzuòá?ïØx0@|‰?lѺ¦ƒ?î$ñқ?*hOñ{Ä?s\/OEóÆ?l·ü²)ɀ4FGL J1112.4+1751¿ë‡V¶}¼@PX£/D'*À;%ö4À< ÷ÞÉN"@››``"@ÄɅðoi?¼Áw녿´ÓœIÍ('?ûdÏÃ!R`?þS…~»÷¿¢-ï7Я¿æÉ	><Þ¿åü8§ç:¿Üg&Ɖ½¿í	}£~?çœÂñAGNbll3FGL J1112.6+17491RXS J111224.2+175131?둱Žÿº­?¸v+
—?œ›GãL7?'ݨ¼Ôe!?¼K¡ÅÉWˆ?¶¿þ ë`?í¡öÉ_íˆ?±øI£‡'ž?Šž‡tŠŠ?£c·ƒBk?¯8ñŒúÛ?¨_ø¿'gº?ìõ×jù­G?bñøs+Ñ?ÝúY‡?ƒ¼‹¬åPÐ?´ੱÿl?˜Í>ˆKØæ?ìëÈ[:¦?£UÑy¡? /í¤ÒO?'
ôÏo—Í?·QÆSÁ©?Ÿè}3j0‰4FGL J1112.5+3448¿§Í*0NS@PâBؤUÀ9L p¸ÏÀÀ<!@ÏÓèJ@Œiƒý%/@ô¡ã6ï?ªÉSE¢Kš?›Wߺæ@$ñÃ&ZÞ@eMÌg¿Ó¼¦Ä¥`ø¿àÉqޔ a¿çˆ	¹½%¿éœ
V›¿éMnÂs-¿ïçâ!´†AGNfsrq3FGL J1112.4+3449TXS 1109+350?ïÏ3~@?†ê\:B?cí 3!"À?]$ðiÈπ?ƒõ&Xm?"'LC‰²0?ï‡#ºˆ‹?ˆð3i%µ?T¨!R@ É?fÀ1oœ?‹¢
QUÉ?‡R Ùd9?îðô_é†?ˆ;8¿¹?~Ï(J«à*?toï/í˜Ý?š-©ð4<?"=Z—éø#?ïØ$…˜?\z˞BCÞ?ZX¿‰F\¤?KÿÔ|†û ?j¯.Í;[?Vnÿ/¡ —4FGL J1113.6-1920¿ïû¶r'@Bë ¾Q	À;›r·®À<"‰†üÞã@|€3>q?ú''Y4?æõ2ôD
?ØbëóÁ{?õú%zãËí@VɩתK¿¯¯EAA'›¿ìä>ÙY£
¿»ÔyŒ]ò¿àMt'yè¿ïúïàM28¿ïÿÿ>¹úAGNbcuNVSS J111348-192252?ïÀeĘ¼ä?"Äߟ?Uƒðfý	?vlo6»[þ?zl!šN%?Ž<©»lû?ïSÅÕô?™¬{y4—)?Wª˜#ñÛ?p"U<n?"µ/"?—Z¥#†?ì0Seæ? =$7/í&?®æ	*ãÞ?‹g!¡!'?·«Uä?›þÝ=®'1?ï3µ‰E…?‰v¸²@?3ËTvc??W',ÃÃ2?™N{þhÙº?‰3è¨J"Ê4FGL J1113.8+1528¿ìS+ºÝ¦@P!¼ÓZ…ˆÀ:õ'R}À<˜s%³@k֒ÉEÚ@Ì_¿ƒ8.?ÀÞº z^k¿¦âSÁÊ?眐úŽ¦÷?ùræ‰âA~?ï›îs¿ìCÑ¡ð§¿ßJ¨/^']¿ßæèArf$¿äw4cn¿ß-¿ÖÅAGNbll2MASS J11135586+1528058?î¦ÿö¶Kˆ?¨{>뇆†?t¡L+Øâ?kØz!e¿?¢ûß«ÌS?§Êûq0•:?íÞn(i3"?®5.ú
?€ýtåë'W?ƒè'»Òy?­ÙÀ?ñæL?¬Ý'Bóá?í§‰xm3?"{€A?…P¨ˆÄò?z]Ò0ÿ±‡?°β+}Ï?'J÷í0ž?ë¦p§êÍ?žaô?–'?¤žÜÇ\?'
",¨×É?¼»ÉŒ¹Eî?™í¹tÄ4FGL J1113.9+5523¿ë.=øU‰@LX[žŒG¡À:Ÿð+oðÀ<ÎeÅV¶Æ@ïÑÃ=­@]'Z
7'?À)§Ù£Iò?¸HÈEÔv?ù@ùª{i-@¨âºtÛt¿çuB!b¦?°'×5[†¿æeçñr¿Ô:Ð`€r¿ãž"Ք¿ï÷އŠMAGNbllSDSS J111356.29+552255.6?ïÉ-²<Øô?v±'-??PÊh!¨ÏÁ?Jítô,?w6ŒÙ)Q±?u8Kµîˆº?ïvܽ®\Ô?ÙáÕÈJ?TŠ½¡æ‹?c'"…eè?·xô4Ô?‹_©ÖmÖ?î÷7{VKÓ?'‹?{õ[?o,˜Ž–?e«`°GX?3}"¤ÄÛ?€]7 Év?ïQ£:ÚY?uã…éèC?'îx»ù?eJÓ¢¯#?Œ:
6Y?rB×Ô|ψ4FGL J1114.5-0819¿àÍAý®õ@G¾Cªy»®À9ԙœØXÀ<+£<±@<Áz^?ü@CßâSG?ºÖ<!ÄJó?ÂL;ÂÎÇ#@­·®W–À@@à$ÃXÛ?拝'uß¿çƧÿ¸ÝW¿ê)!¯íï¿ìäÐ.Ë¿ï¢£Y6¿ë¾hêAGNfsrqPKS B1112-080?0•L?'ÖoÇæ,?ÛƯ苌?~ÖeÒ¥É?p_¡ŠÎÛ?lÀ^@xaÜ?îBÚõ×?¬Â{–"?'A…?ŽAË1'ðv?§Eæ|o]Œ?§ÜÛ{Ÿ?îö´B/Ø?ƒì€Tê•?vPy
ã!?gã.Œ¢æƒ?›•]ÔA<•?¿µúù!Ñ?íס°óø?'íê¹ýÜ?£4E'ÊC?Žô <ïs›?ž£>½ìyÍ?'D	‹A¤'4FGL J1114.7-0248¿ìG'#©Rt@J¨~8ëÀ:EÏÞ²À<)œ1úN@&¹¶ðl@òÊ!÷¡?ÃúûHáb?¶y"˜€•?ð™šäó?ÿàTyá?ÖBˆCa¿êÉԕ*™¿è±5Ý\'ü¿çӄ¼¿ïý¸'gù¹?ÊöÖ-ɒAGNfsrqPMN J1114-0248?î×÷0Ì«Ç? çþ*I»?›ÙX¸~ÿA?¿¼àâà?'O'[×Õ?€ÌtT2ÍÆ?ë›ÿ‡pjê?ºN19O?£?é;ϧµ?ª¼¸µNö7?¹€&"ÔÖ?³sÛÞR?ë·@øº˜ë?Ÿô
‡˜O¡? hÄ藀I?Ž÷ ¬àt?º•ÅßxŠ?™#wžÈ?ë¤[p"??¢f²Vb#?®G%ôh?˜Hκw?³¹¡kõ¹À?™ÑÙJ!¤4FGL J1115.2-0703?ÑÚ'ä@HQ^	À:XaÀå8À<Lk"ÌÐÿ@ò;"™¦@@"Eð?ºÒ6™A?¥&¨$:¶¤?çވì£+ê@ÆâCV–æ¿æƽêî¿Þ.dß¾—¿åÎÆ×ÀEÖ¿à-î$nt¿çéŸ"w¿ÙÀq_=ÓAGNbcu3FGL J1115.0-0701NVSS J111511-070238?ïgÒZlˆ?†üéßQ«?`"r.cˆµ?S"`jj?óFjEýñ?…àÙÓ÷?ïˆþN?‰g/ÕY f?KÂýIš%?Y†ñO¸°¨?Œ@Ükê?‡ÝÕeD"?ï
͝†?•'ªˆ¡H?kP5™‹¥i?VúÝ5ׄ?šÜX¹,º©?ó½Ém?ïK|ôþ.?v¢þÍ,?u!Røk+?^ŠO¤»¯?'NY|%L?s£ßç#s4FGL J1116.6+2915?ì'<Ë.ß^@QB­­ê‰À<Kl»êý9À= ¤&ó@#¨©Úî¤?鐗ÈAî?ép›Þî7?ê~e`¬é@"ÄæN~@üiÙ¿ïÿùSt?ê‹ùæ/t¿ØÞ|øy#?ï¡æڕl?Ì«IYæ%c¿Ð2":¯ÔDAGNrdgB2 1113+29?íÈ.ñ¼œ?´/¹HêÙ?˜–n6Ùð?¢úš¡¬?§1ÙÈõK?®ø*K'?ï@!êo™1?¦ZÁ°Uj?ooô""~ç?"|½ëãN?"
Ä!zj? Ä7¾º$?ë³ÒR\7Ì?£ÚD¢:¿á?"ÐLŸeª?†¥ŸêÊ^"?½-ZEDÿ¹?¢Ú2×ñö?ïý Ð\v?" o3@$o?C±'ç•VÃ?^˜^È2®ˆ?›bÏηƄ?"yãüµüS4FGL J1117.0+2013?êk€«zÜY@P×j~ùÛ#À8úùåܞÀ;ï*¯ÖòÀ@9 Va¶~?ÿH"¹7Ē?¤œ|^0ž?Q~'œRç?±"÷¦À½@±pÿÇuö?ϗ#k"ù¿ããpè gê¿áE†òÍè¿Õ掿ËÝd¿äο€³ï†¿Ð.feÍxAGNbll3FGL J1117.0+2014RBS 0958?ïövRGåH?TJ½5Gr?˜ÄÅHï?{<Ú]î?QIÏ#àà¨?RØñÆ®ðô?ï²)Áã¡?'¡ø'Â*??ÌzßZK?Q–¯·*H?'}'¿(¼?´¢[Kþ7?ï¬òr?…´=¨Òß?gú0ªÉ?UTν§?›x¿©<<?"¢ÞÒr/@?ïðï	‰?LĘ?0íú«–?"c!}û®?[Ä¢ánAù?IìÁS0Ié4FGL J1117.2+0008?¾ÊÌƱn'@Kcí¿‹›ªÀ:÷k:
½ÉÀ<Š|@Ã?@ ¤É'PÑÕ?üº¡6F
+?Ë­=¾§p?®|>>ÿð?â®q,"@µ+‹¿îÏõ@‰]?ïév†oj¿Í$¨ҿDžþ²"&›¿éÃl2š‡?֖K›ßÄ÷AGNbllRX J1117.2+0006?ïN~ñޞ?;xAÍ@}?P×pSÀu?I¶Ä¬ÅŽ?•"Ç\ˆ%?Œ©gÈ+?ïé*bû?†q™rÙó?Ez©ìTk?VrÒDÄ>?‡.\Ú|
?…º!—?íìúÍAH—?'òa!xJ?€y"ÞÞ|Ð?xŽ&êlY/?­íô3×V?é!xžïŽ?ïE'6¯?{ΟÁÀ‹?gèÜÃè?V›HGÝ+Ã?"R¸»Î"e?zGu3ÙÌ#4FGL J1117.2-5337?ïÐãò+t@ÐO±;`À9ÜRX'hMÀ<HjÒܱ@¤ëg†ù?û1GÏ¢j?¼+‹tõ¡?Ì´ªV«2s@…Ìe÷@ºe+'÷?î©¡ÙY"¿ä
~q ¿ÓØe1]¿Óޖ"ì"¿á̈¿V"¿ïÿ'âH	.AGNbcu3FGL J1117.2-5338MGPS J111715-533816?ç@(l±!;?Ã[|*¦mÑ?Àó6C«?·ÕRrŽ×¦?Âßk÷Ð?¶ïá3©?ÕÑÅtŒ¢v?ÇYàî~YÐ?°8çY7(?³0«v‹Q?ãZ'ÉÄ?ÆçÔ;û?æ(µg?¬ÂZ}õŠ!?»Éƒop2?¤b•"zrÖ?É›sïŸË?£¯™C·ýt?ä;¡þàûs?©"ŽÈÝ?²#f£'&?•Q¼Eýë	?ÒÿâYyÿR?ª0Ds½§4FGL J1117.6+2550¿êa·šÇ¨@Q@9Õä¤À:tu;ÄÀ<šk‹iU.@úGtª@Í]…U?º]âžÆ)E?Žê¾¶oÏW?Ôf˜:@YYBfê?î†òBR5¿âÂÖ>e–]¿ãæÅÒÈq¿ãµDD¿æہÁ
̸¿Ù¥W½×žAGNbll3FGL J1117.3+2546RX J1117.6+2548?î¢	>"?˜˜í¯ ]Z?wÙÐxŸ³Þ?jdÅm¯!Œ?¢ã"€X A?—/é(ÍnH?ïSæ,¥ê?Žr¡|¾T?W—és?dŸÊÇñW?"AÂt"=?Œ'ÃʓI?íÕüÜ·-?'uä(µo?"F¾M8Ív?r4k£8¾?­Ž'«FYÙ?…ZÙè>Ç?î],Œ´ñ?†oŒbº§?"¼áG*=?wÏ
®œ? ŸXÄÜ?'S¡Võ4FGL J1117.6+0217?æ8ôxë׳@LBŒi/nƒÀ:Èût€À<])4¬¯÷@S¹¿~Û}@ ¶fXúm?Ä\HUYMÏ?B»ÆÇúl?¡Þ.ÁUí•@gÕR­Kþ?ïtŠˆ×¿â'~e'¿é´*¿qD'¿ÕØO¢T©%¿ë8ë¹4¿ïñÂàÍ=AGNbcu3FGL J1117.7+0217PMN J1117+0216?ï"uÄÝt2?‡‰}Üõñ?d°ç€ˆÜ?\O¦­í?‰¶U'Ñ¡?…¨V'–¼ë?ï•Åíž[v?‰˜E.÷‹Ú?FÁGy'YV?WöñùΛ¢?‰"p ÐÌ?ˆZˆï;B?îSKqb¾ª?~Š–'?zP¯¹öÎ?iÆÕBÔ¿Ã?§6ÓÜև?´9q ?ïL7A9Ð?~ê]HW~?|Q'ÍÚ?g4Ìþæ?•Â17%ƒ?zgÏæYP4FGL J1117.7-3650?ïì'n…wV@6Y~™cõÀ;òø°€fÀ<"ö(æ©@Ҏqó7p?üãx«ˆ¤?Ôo›-îOÔ?Ó.¹PïÝ?ûUȤI @}´üvˆ?ïÌʳíض¿é0ç"øoé¿¢è&šs‰:¿Ý[5ZÕ¹…¿î¹Þ]˜âe?ÕX@2õö'AGNbcuNVSS J111758-364918?íí
'¶?§«æSõ!?©áI½]?wÄz}ø,?­9êf·?¦¥¾›¾Xý?íÙ=ôm-?§ÅB]ʏ?…â‹é#…°?Í"yfþÛ?¬ó‹pKÄ?£áX§£?강óçÓô?¤Hc"u¼Ä?¨ó˓®?"0«Áþ^Ž?¾j–ê^^?Ÿ¶^ÙÜE?ë˜Ã3ƒ¬?Ÿ)^Å%Ï7?'·3,L¶?ƒMPSôâ?¿8šðÏk?œƒiîSjQ4FGL J1118.0+5356¿¢ºýÈfbj@M¬ÿ§ëlÀ9†S³Ü;À<"û¥'l@"J"ú?ü‰ÔÊÈÏ?­Ÿ¶¿Zð?²?Mȵ»ä@_íQx™@‡k'–Fÿ?ïÐnýäœÍ¿"
ñ)¥…¿àWŠáÅ¿×h^ùŠšù¿â.î%)¿Ú½_œr¼áAGNbll3FGL J1117.9+5355NVSS J111757+535553?îÑIfóîÑ?'úôj':ì?tÝÌþ'Ì?jiß? h
×!@"?'›þ—YE?îÞVÃP×b? »\7A¡°?w­ÂꦹN?‡"<nÆû4?žI¶Û;eŠ?™8÷f¨?í
þ—¬?œ1ûWËY§?'9Vô?†s:éb?²ñK
±ý§?–ˆQƒ,?ì²Q¬­Ã?—ø¥/i? ²rè'Ÿ¢?ˆ>éYuؖ?²9+.Â?–ãZú4FGL J1118.2-4634¿åÏOë>–­@*«nø_»À:ZëÞàÌÀ<3ˆ˜`´@¬Q'M›@TªFJ?Ñ4òÛª5H?Ú$&»U¬@1[µˆ@(t,vÖ?ïövêB(™¿k»Ý2Âí¿çòCŸ'Æ¿æcçeÕFï¿ç]13~²Ž¿Æg³'ùÄýAGNfsrq3FGL J1117.7-4632PKS 1116-46?î|jF? d‡Íq?›ã²R˜?˜úeȼù?•j:[_?'@7ïh?ë>/ãànû?ÁÉôÙ-UŠ?§tóŽº?´eñ ç?ºˆF҂ÀÑ?¹!ͤ¨X±?é2é/A?ªv÷>‰?²Ëš${¬?´ÓXdG?ÁΌ­&?£oðê›ìz?ë_ü?Sò?¤wíY€ô?¨óó\0<]?"tïrÏÛ?¸†%gíBF?¤%È+ëÄ$4FGL J1118.2-0415?ﮃ¼ô£½@I²@(äüÀ9¶<ËbjÀ<z¹ÚÁ@ †ôü@Ù@ÍG¤ç?·ë'ˆþì°?¶¤?	ˆ?ù+õQP@|@BeU¿Ú rÑ®³Ý¿ãá01 3¿è—è¿qšw¿çœ'aï‰:¿ìÓfQÒ[¿ï"Í®oêAGNagn3FGL J1118.2-0411PMN J1118-0413?ïí€4db?a&³ý7U«?E²²°ø‹?FEPð³k?Zç¦?'<Ç?\ù¤"€»?ï§Ö'Óò«?"¯°œÒßv?B ùÛg ?V!IT-?"àZûežÍ?ƒŸ¦þ¸'?ï'ʂÙK?éÔÈJ²?qyXÛgÂ?_¼›gž'?–¨Ymü«ç?¾<uôyÂ?ïïšøI‡?MCLö™iz?<,sÃ2n?0/ôKÅxª?Y¾ò|%+?IîM=xä4FGL J1118.6-1235?ï%7‹BÏï@F*䎊qÞÀ9öñûÀ<;Æ*\}@ÛÓöeM@Hæùž¼ï?¼±;aU"?Âj‡ÃŸÒ@	Ĩa³@8÷¯#™?ïÿÿÊPË¿çîG;'ô;¿ê|Vþ–¶¿èӃÕâö¿ãÏò@Ϩõ¿ïþ,UÉ`1AGNfsrqPKS 1115-12?ïçe5t™±?e$ü)A*?Sˆ<±œ×ê?Wê¡4h?]­Xe/Æ·?\:¶Y¹§?îâX'[ö?ýÏûC'8?qp£'Aߛ?€H¯)oÃ~?ŸXÒ/ðÄQ?™æ¬–N:??îš%«™?Œv"Tnð?z^_ƒó~?r"ù½5Å?£ÙV"°O?‰/ÞÈ?îpúpÞú?.<¬?™ŸëÙm?‡¯¬Æ~Ò<?˜@Æ%ƒ³°?~g.u4FGL J1119.0+1235¿í'Ùž8Ý@Oø·`,'À9íÝ{p¹¦À<Þzt:@%ÿµØ>›@=ðüVþ?½M6êwØ?Í^#vҚA@3xî(g'@
~w)W<¿ÂäÏw÷ÞH¿Ý8e˜º¿çÊ3ß3W¿ê¿cW¾-¿ïþÖj€˜?î§<_VÒ AGNfsrqOM 127?ïc¹b?­‹MȓwÉ?"p:ºÛ?£Ühú9\?'¡a,¡Äø?•˜]HÁl?îð{õâD?¡åX2?qYû]º›ì?€þN$CÇ?š†õž?žö=­ð]?ís¦Vv?¡~—£0äÛ?£NÈgy?•sÄô¬ùw?¬@)¬Ò1?•öNÍ\?ïÉ"œg?‰Ml#³Ý?|F!mÞ­?m—<yèò‰?˜
þ˜û"?†
<&~#4FGL J1119.6-3047¿àT‹ÃÔ<@<ÈæŽ>óÀ;c…LXžÀ<´)3Õðb@"/sš×\?ü8ÇÃ?ǂ´eLàÙ¿˜Du?Ò¼Ú;uL@'®¨—›¿ÕÀæå|Æû?ïÜE É
пë{;	ÁJ¿µ59È£T¿×ö‰Ÿ%Ÿ¢?țt$¿ýÜAGNbll3FGL J1119.7-30461RXS J111941.0-304652?ïxÞù½á?‡†}íEöl?QNû±"G?Jþ5æÈ}?žbgiß?‡-ˆM¸jL?ï"D5.ìÆ?ˆ™'ðJ|]?Dü…G=Ow?VU<á+=<?‰ß*_Ðùk?‡$í/DÙ¶?íì<úõ?'ƒ`¢	nN?r@kod?^Ùh¡ÎZ?®öB
B`p?ÑE"ÅP™?îY?	±¯?"®xG:Ò?lñUäÉ©ë?dopw-};?¨ŸF±J_?"¶…DFį4FGL J1120.6+0713?ï€/úˆ`¦@NV0U2a|À9ä(rÀ<P)Ôà@˜à¯à«?üÉçÅv—6?¾Fa8T/W?ٟúdŠn@XÿI Û@ˆj$aY¿éŠÐ=š•B?Ð6¢~oœ›¿×>adžæ
¿â¸J"xÈi¿ïÅ<¡?ßjÊÄ^êAGNbcu3FGL J1120.6+07131RXS J112041.6+071335?´']î9Ú?²u°œ÷?ì¾Rw'JÐ?µøUx~?—»g•ý¾¤?–¶´¾*Ø
?Ëör'Äd?Ë?2¤#?åҐ{4Ã?Ïbvýï
#?¹~›Ñ?²—-ž|T§?ªâ.g-?™Éæ_$5€?ënŠê-Ð`?¡¼>܂­[?·'¬]æv?™Û%$ko?Ý:×s…×g?·éíH†¹Ø?×ÂD÷<÷ç?ºÄ(IÂ1?ÆÇ*zae?©w½×²Ä]4FGL J1120.8+4212¿ÌF ;ÁU@PŠk΅3±À8ÁA÷TðÀ;¦. |w@ ¾ØÈ.?ùÀ¿xPt?¤wÉ¡Zii?§`®>@eŽšbv@tmoïüþ¿ç'E'ƒ¿Ï²¼•ÇýۿՄ½A¿h¿ÕKí^'²u¿ÉHY`™¿Ñ+¼üKAGNbll3FGL J1120.8+4212RBS 0970?í3Ær¥ñ?¬{Ôä_ñ€?…žCç%#?ƒ»u
çQ?³®íïòŽ?ªs7oóÏ?îk–@PˆÔ?ªƒÐÃÕP?ƒS"{ØO?—¤g"ñ
?¤qÛ|¸?£˜\Óªƒ
?紪ɬ|Å?°bfRÈ¥?œ)+l"7?ª‡aM?ͨ43àˆ¦?¯e"ñ>ƒ?æ·ã˳Ý?°ÞÆÍéj?¡ãWêù?'âcã<GM?ÐUp}šæ?°Œ"n§/4FGL J1121.3-0011¿ïÑÀeúõn@K"Q´þÀ;ËñºzÀ<œdÐd1@ Hƒ}Îaø?ÿ"à°«.?Êϝ÷øµ?ŽÚÜs͛î?Å£øSY@ҍٜéÛ¿ïÛO¡ÓÏË?ïý…Ò<xV¿ÛeD¨P—¿ä6"Ü¢¿ÃÛ-¸Ÿï¿è;¿(Ÿ[zAGNbcuMGC 0019706?ï£Y¨Ó$X?"ts"J÷²?P×9KùÓ?Mً»?…®¡Ö
ë?ƒr·&Ý?ï‹x^½Š'?‰A¾Ð€:ß?Bò5†‡ó?QÕvÆ֊E?‹òÈ=E
ç?ˆdûç
"?íåÐJ§?'q9?{Áñáé?nLFü7Ö?®6)Áß4?;°Á¾h?îԑí<?†×ÊÕv÷ñ?e3£%¯uù?]N€µï?¡c­ÎÑFà?†jř1¸Ø4FGL J1121.4-0553¿æ%ÖқT@I9PüqÖÀ8¥Q­DqÀ;Ï×ð}ñ@¡sÕB<@x"¡¸?£À–2±Ù?Á£~õ©dé@Sžã…v@ƒaòåæ¿ÍýV
㘿â°]ˍ1¬¿å*Ú~çÆ¿æÀ–]¤öÅ¿íƒ|V'³Ì¿ã$A"àAGNfsrq3FGL J1121.4-0554PKS 1118-05?îœõ-Ú°?¢Ï%ì9ê›?Œë™Ø®!?ŠÂìCSÌ?ë×íXRÓ?žChµ]u?îö©ˆÄ?ŸXyB™d?iå+¥àU?t>µ¹w,?î)‰3¼é?œÊøÓ%þ?îð¤Úž?£¢ôŒl?t¹p¯?‰Ë2Ýu±?¨ò³êùû? ã±Ý£Š?ïŠFU-AS?uù9!'¨?rŇzŽe,?b€õH"Á?"¦÷hx[?qx"± 4FGL J1123.1-3233?êóÆ,¹`M@:¹Ñ¢£YÀ;–m•/À<žÉ¬†Ü(@Rž˜†ôü@óý]ŽP?ÅÁ¼"…ù?‹†ù?Èòüvރ®@‡A 3fµ?î=ï^òÿ'?ï§$f畦¿ì)õœÏ®ÿ?"×Bz+Æ¿ÜKóÞßsî¿ïÿõž}.)AGNbll1RXS J112318.0-323219?ïÒùLú7?q3ۃ£.?J­Vv~?Vh÷‹ÙÏÛ?s-·"
ö?nÄÁwg&?ï»TxˆCÂ?'ÑÊpJú?<ÿ±™Ž ?PQy–&¡?€BäQ"š*?¡"¬û¨?îE
?'<æËÓ±?v½±oص?f¶³_ŽÒ|?¬ðìñ4´?'()•Åµ?ïÏ8ö?xµF…¬à?pvOQ¸A?e¶W…þö?† œcU¡±?t>Êr©–24FGL J1123.4-2529¿ëÌ$á
ò@@£Þzt:À:´É.4À<Q¤Æô@?ÿòˆJ¼½?Ë,Xãñ×s?Ó¢šÛ¸ù@j[¾l·¹@«_ð«y¿î´@ÿ¤n?ïý_;Ϲç¿âFr«G¿ã¢$'–H¿çêèÁŸòú¿ïÿß~€8 AGNfsrq3FGL J1123.3-2529NVSS J112325-252858?r"ªŠ?z| TÀø?`	<rÊ­?X""Š&Ë?y2"5¢Õ¼?wC§áo!ƒ?ïrÆü‰wB?Õ"FY?ZóéS?iÖoƒªÜœ?ïßà­£?Š^ž25]?í_¤
ß?šݾ±†ª?—´ž?‰ÁpUÖæ?®xT¶¿S?"";Ù´?ï±²ó}?|P,xèhØ?|8Éñý?eËôþP%?•û¦_k4?wE?ӕ‡x4FGL J1123.5-6418¿Ã™E˜:ŸÀ] Å®À9ªkµZÀ@À;)Ì¢Ûb@¥'—H±@EKc¬?Èaq	,¤y?¼ðò›éU?øyìU(Q@¡¨ä»+?ïÿP3:¿â¶CÞÒõ¿æä%®æ2¿ì	tÞNTw¿è(úà†h¿î–JŸ‹vAGNbcu3FGL J1123.2-6415AT20G J112319-641735?ë¼»›?¶3—ÕF¹*?G ¹¨à?@<n®H6?ÀõrΌ¤ò?¶$Š"!âi?ããsˆŽËF?ÊRwxœ×'?mLáåö_Ñ?€[h¹ôò'?×þ+|´?É÷¼VÜ?çn:ýqÒ?­j€ºø©?˜1ƒŸBí?…Cönw¯¼?Ï@ã–PtÞ?«¯"ìýÓ?ç±{x[‡º?«ìµ¾–+/?{öTóIáô?gé;›£?Ð-/»{É?«ª1¸iJ4FGL J1123.6+8028¿´~F
ø³}@AótÝÛÀ:Øý›²yÀ<ÍK
P¼@o*|«L?ÿ³vŸ™Û?ËO äüïT?Õê{´V^@>À·pD@ÖèÚt€¿î''¼¨'?ïùx&'JÈ¿å‹ZÜÅhT¿Ù'D:Ât¿î­¿jäz¿ïóHa˜¡LAGNbcuWN B1120.0+8046?í©^ãû¨?ª9ªŽGa?œ°Îa«¼&?Ÿû^2¡Ö?§ªž
g'?£³n*H¡*?í¨"ßãƒà?±¦ðŒªç?—†¶ÅnUã?£É·¤Cf?©ºvŸ–í?¤K—Æ#ò§?êÌñz"œ?¤àØøB?¬ëé$P&?—=#Mz°t?»)Câè…?9¹xš?ë¯$gWí?£;À*˜=?¶±jËæS? í}Ô¡]M?§«ˆ!½Û?Œ[D|ª4FGL J1123.8+7230?ïoچ§W%@EŠn~bÜnÀ;œ®¶aP}À=¡'Œ_@!¹üøä'Ì?øÃæÄŗN?Ê-˜),A?ɀ1©k@óH+è¼?õöA»6L¿ïÓèë"³¿ï¶R¢dCv?ïÿÂWþÅ¿×î]@L÷¿ßx`cíæ"¿È*ýD8êAGNbll3FGL J1123.6+7231RX J1123.8+7230?ïÈíFÔÆJ?tVoù(?FŠ]Êy?Gº¶a×?x¸	ãš?rÙ½ë?(¾?«}b8ï]?'ð8`\?ºÁišë?ªæš:0¼?¦‰D2rr?íW#f…
t?–ÿýäw¤"?‡Šµ
Xú?0Cf>d?²eu6aB?"½Ïý€Ö?ë
"ƛ8Í?©ŒÅÑeYh?'/3GaÙ?Ž@jt–œ?Á¥Ž|¦á¯?§à">)"[4FGL J1124.0+2336¿Æp×tÃJ@Q~Æ"§À9ìú'è},À<-:ƒ‰ŒÜ@¹ö¾ëv@Bá¹Ãۍ?³ÌÕ±!öu?"Tµ ¥?Ô4ªžP8@ž{Fó.‹¿í'ó*ö?ÌÒE݄Õè¿ç$ŽŠqÞj¿ãi!Œ—¨¿ä
':ƒŽ¿çø— B•§AGNfsrq3FGL J1124.1+2337OM 235?ï€Ð_éÌ?¡Õ´ ²¿Ó?p®TCb­R?iSè>b=?˜ÄPã*%?¡~ºõk›?A¶jý?ŠÝ-ÀȨ?UK/¾=U?d£Ï·ò[?Šñɚ¡¹?ˆv"Ei?î5%³®_{?"CQÑ?ƒ^Qx
Ð?xN£4eÃ'?§Ög"L?9vež<l?îë˜û£í*?´8ŠÅ³?‰ÆŸŸå©z?so°¿Ä*?•©»…û?{Azf7º4FGL J1124.0+2045?ï
Óyus@QEy¿ß~€À;Ù¦ÏãÀ<¢­\Äüõ@ iZA"ö?þ*ål[?ÍÆ^ˆ¦?´¦ùS"{?ìzšï°@œ¶ü%?ïã_0пÔ3Éü7ôc¿ßƒ~O;R¿Ù*ü˜lrð¿Ý|¢gô[¿ç\ß¶´]AGNbllSDSS J112405.35+204553.7?ï°:"î"?||
¢µ›V?@¯²i™?9ÃN}~"C?'憢ô0?{¿¢ÿ?ï~¤…î7É?‹ˆ©œ5Î@?KÊX´?Tló
l«ü?ŽÑÞæ̝?ŠŒYT?î0˜Ö,w?zH'ï<?r¯ZŸ« ?["77â^"?ª "^§Ä"?²-Cª"	?îD&âáÐô?9"ë"Eb?~ïy²T&?oUª¶Œ¯?§ß¢› †O?Ž&+×é§l4FGL J1124.4+2308?îC»#,*@Q{€Ü3rÀ:ã¿Í
	nÀ<]RÁmóù@T1I#4@bÁ–8?ÆM8`C¸?A±=é/Z@È1ÉPÁd?æcq>†£s¿ì>!£¿¿çà¾áý‹‡¿Øˆ¯üÝ`Ä¿ÞyÌÑý8¿ðAGNbcuCRATES J112431+230745?ïÁ¦ÙËö?|(±^òTU?Ix\ˆÆ¼ž?D%¢Šçÿ?{ý‡ˆì
?z®\'KÜü?ïoÈ=6ç?Ž&t¹'ÛØ?LȒªšx
?Yã16=²?' «ƒOt?:Õ|??í—U(à_?˜MóQ]¼?zu¶à6¦?k©ÖŠÑ
ð?±œO]?–½¯VÙ?î?L[lé?'—ƒ »?}­î/ÍU°?n
íUù·È?«MtO†Ç?'.^NòN4FGL J1124.6-0809?ÝkL }ʗ@Hv <K	êÀ;MFÚ°À<tò ›ìZ@ AêÜs@…Ù ð¥ð?Ï?8ÇǪ?£&Î 		ê?Ք˜B±@‰;¿HÕ²¿âBRÑ^,¿æbP1ò¿èð›.£¿¿cŸŒ¢»+¿è=…Ò<xV¿ïîåüH»[AGNbcuAT20G J112437-080643?ïá+é%,?"E]%­¤?XDáÆï?R	CÑY?ŸŒfzÛ°?"ÖŒ1v[ç?ï\ó€Ïd?·œ‰â3?PGÈ}>½V?[Àïpà?"]È'¥?Biëtõ?íÿÓâq€%?"Ÿ87\Ç?xÇÀª´
?iNWSõ?¬éÉا6?Îò¼w9î?í²IsÌÿK?"Ícó$?{·QÎk?n¯,=ÆhÀ?°²BŒ†xÅ?"+>¨Ë
O4FGL J1124.9+2143¿ëםy‰?@QgÙŽuyÀ;
)Ù]ëÀ<³ó;Ì_@r,…o7@B\=îx?ÆÝ«Â;#m?¥ùìj¡ßc?ã|楻æË?÷¼¿øÓç¿íxmÏç3€?ïú¬Î)Ä¿å{ ŠN£¿Ô	.3ð¿çnýäœÍ¿ÆjVJpKAGNbllSDSS J112503.64+214300.1?ïIß7Š7$?"m?«ìCÙ?T»zUwº?Oá…§–?•{=WÃØ?"P¬¬?ïWô£c—?—?
«r3g?h˜'WÀW?s&âù?šÿf¨•:?"ø Ã­½?îšiù7Ê?'·þ:bœí?|Ó¼²¥
?p•ìI®äÚ?¬+áÊ*ŽÂ?Æ"'q…?ì«ûõIß]?—û5Éo
?¤ƒr*IÑá?Ž¾†·ލ?°^g@Œ#?üg4œ"p4FGL J1124.9+4934¿îri¼(²@Ož@ÈG,À:ыxn§À<5ÜF½S³@ò5#ù.€?øNŒ¥•P_?¹ÀÖIxD	?Ã-ÄßB›0@)ÃÂb@
'AÜCb?ålk˜ÕN|?ïÝ`='l¿ÍüÖö¿Õ]°ŸÅ'¬¿Ôbºõ8§¿å_ü?EöAGNbll3FGL J1124.9+4932GB6 J1124+4933?ïÇÊçyeÉ?tÌtÀÙÑ?n˧Kù֒?k]Ðftþ?iiq: ^Ó?d²XìœHÚ?{mŸ'?‰¦Ðð#e?S
¼@k!?bq¢G¯_?‹ºIœŠ«¼?‡­Há?îvÆÜ9}¿?'"
Ú¬»
?'ã⎚Ì?±…ÒAw¸?£Ú™˜åýA?>"³¸?îjõóÕú?'ÍQ:C´?vW³%«å?k×$H‡'?¥Z<
#Ì?'<€¸ÊÆV4FGL J1125.0-5804¿ìpBM,ƒ—@ ñ,'¦7À:M¼)çZÀ<zF"b@!þ"à$Œ?÷';ý?ÆûQš|m?Öw¦)ÊÔ¥@‡‰Fe?@K'à—ÚÓ¿ïýVlô!¿ï+Bn9™?ïýÀTïEž?Ð/ûZԷӿ͕c>"¹†¿ãϺ 9qAGNbcu3FGL J1125.1-58032MASS J11250388-5805404?ÏÆÂÑöí?ÂÓÞ~T-?®¬–Ð0Y?¥Cúšió«?æ#…ÞVó?Ã[sŒ×Ņ?Ú`eúŦ ?ͦVI"?NùÞ^¥?±‰>ÒÙ®Á?áãJŠÎ9»?Ìcþwªg?ß¿=O k?®¸=_ÎI?Ä#ÂÛ¿*¤?§‰;­D]F?Ö.á'ÑJB?ª÷'åäY?❊/gJË?¿Ç;ˆ>Ð[?ŽÂ!q?'?³†×*!?ÙÔÛ=#Y^?ÀRe)(4FGL J1125.1-2101?ål¡©]†ï@BÁˆ†aÀ9îÚøººÀ<:¿:=°@u,ŽSj`?ü©—"ÆÔe?¾OÓ@É¾?Ä÷'>]@Ôi
à"S@Þ跎ø¿ïòx6?ï>Áï#9¿Ò´ßñÙ¿ÝÑ·D¥¿ä¬;'}E¦¿Ýdæßr–ËAGNbll3FGL J1125.0-2101PMN J1125-2100?ïÞr¨ìÛ?c×	÷¬ê9?\g'"®ô?U;4"×?cYŽ£¼"¿?Z–×·­]õ?ïR'æ¥?'‰æ«0Õß?d!mÒa?rJEyÜ?"+ù?èß9?¡ÚEK?îé©9é?ˆ23?s\%ž<I?lI ¥×x?óÏv°?"åÜQ4sî?îl=Ó¦Ï?†ä˜Úd?‹Í‰@z³ž?u)/L¸U¹?¢HÀuxV(?'°z;€Ýa4FGL J1125.5-3557?з¼Ý–t@7¾ÕϪ͟À9Ý¿zÔ²tÀ<:b'œOV@"A"ßÿ@ñÜPÎO?²ãÂË O?'B@c®Œ?ÒÄ«Á}œ@.~]Ë?ïÿ"g3¿áß
Q'™Ë¿à¬1¡¸¡ó¿â7´lƒ¶Ù¿Ùˆi[
lпßr&c$ÚAGNbll3FGL J1125.5-3558PMN J1125-3556?ïՀ¢™¯^?~@îÂ2ò?9âÕ@õƞ?5≀½Õ?s¡_ôû?}(¦pã©?ïˆ?w'?|j ¤qSd?/%4_i-?CÞÀÉÐ!?yC¶ÓÈõù?{4`€¥¢£?î÷–-ª‰µ?†cŽ'´¿¶?guƒêl¹?V¹yÁº?ž+kš1{Ü?…R˜9hŸ†?°^¨ë?n|Øé:V?Qï¦WÿÙ?=zm7+ÒÉ?ˆ_UäK?m¯ñsÞìË4FGL J1125.9-0742?á_xn@H¼ƒBÙÀ:"CïCÀ<_^4h½Y@ò¿ûƒ@ÖqáÄ«–?¿cÌ®…?`†K¤«?´É¼L!?öå§×ŸäŒ¿ïÌ7å?ï~•Òd¼B¿ã…Lò!¿â¾œ)¥ì¿ÙH¯œ:^¿á¥·]®1AGNbll3FGL J1125.8-07451RXS J112551.6-074219?ïgâtöG?Œ((¥¾ñ¢?cA¤Î½§?\­g{ýÝr?·!ÜÇ_W?‰ç7ú"Š?ï"'^©‡£?–hú‡)
1?cÓ@ÙáG?o˜à
¹?™3l'âÖ?"aÆ5uÞò?íŒ8¸¶nk?"‡Hm(€~?‡²X¾¶?wFÐ;Ëí?°»Ãï4µè?'"0†©?ìð³hX.@?•i~½¸?M)ö™´?ŠkðŽóZä?±'"²Àç™?'ºün)'¾4FGL J1125.9+2005¿×âu´Í @QNµ ÝDÀ:ÁóTöÒÀ<m2ûÕÎÔ@ØdS爻@Âãú滋?¶h#ªÕM?«¬d!'¡Ù?ó¶îßFL@î[R×é?í.öWà'¦¿'ù†Fß,¿æôxþŸ3¿à2üâ>N¿æï¡ðÖ¿ïÿþÐñAGNfsrq3FGL J1125.9+20074C +20.25?ïYÙ7<E?·•y`?jj0"^C•?Uɸ'–£?'žÔÌ®Ù?´¼‰'3?ï¢ìÜ´Õ?……¥Ù?Cˆ€D$ô¡?S–LŠ÷±?†C¼Ä{3?"nöp›.?瀞¨Y?€ÌïÄ&?q&Œâ<%?e¥pu?—ÁûÔg?}cªfÙK?ï´"DºÎ?g®¤a×`±?j袆YÐî?V-¸ïH¦?x}šu°Ð?b´.¾•ß4FGL J1126.8-3829¿ê3\qH@5uX!)EtÀ9¥Ìô9ù À<>ô±d¡@÷oV¤ýP@|½ÀÀO?²Êà
œJÏ?¶˜ã¼'Ž@aÑü·v#@8³Ík-?Á4âö.ðÙ¿ÝEÓÿqá¿æs	¿àwy¥Œ¿ä3ZÖk®¿ïüev|^AGNbcu3FGL J1126.7-3834PKS 1124-382?îý閁У?'«¾f؜Ä?s§¤1b†`?i9LÊÀn?›Xä#mIû?ªse‹<a?séf·?¤ 	,'×î?€;Öñò¢ñ?'™YÞQù¶? Æóìë×?žYʲû"•?î5Š=V?"|X¦~¡?'·8«fû‰?x'¾ÒÔ˂?§ù'±N+À?ÓÆ~
?ìÈ×Î @z?'£'ƒN(ä?¢áQ"a??"\,cä«?°H¹f;˚?‹£«C±4FGL J1127.0-1857?îã9bn¬}@Cɚ¿3‡À7s;dZ¬À;Y–¹‰$@vú«Ø5Œ@¼ô}þ•?"ÕÊCÒà?´ägH8¨é@!ŽGUÿç@ "ŒdQä¿Å`Ó)ˆ9 ¿Þožˆì£,¿ã‹à)÷¿ãèJ®kc¿æy2Pµ$:¿èžÎÂpRxAGNfsrq3FGL J1127.0-1857PKS 1124-186?ïÜóÀ"8?døŸÉØà?<!µTN$?79zíŽ?oˆ	Mò²?dG
â)(?ï?Õìãý?¡5‰ûYè=?aŠ<Iï?|þgX×Û?•Ô>{÷? œ«ˆ;?ï\N"y*ù?…÷"FQü?ya Û@Î?vÃÔxü}?Œ;Ê´ڕ?€Ž¯ñÝd?ï÷ÑtÊaö?Cÿ¶Óu
?Àçywö
?DŒÚz›»?LâçI'Ò?Büõ*4FGL J1127.4+5648?êRóÓw@Lbك"t—À:KÝþMxYÀ<ªþÊuÚx@
ÀaÖ	@mñf­´?¹A]˜a‹5?´ü‹+lÀH?õÈbŠ8ӆ@/Vôk!?ïÿäA2¥D¿è"d
ƒ ¿é3)Wèb¿êSi©¿æ€››ÒXþ¿ïÿþªJlAGNfsrqS4 1124+57?ïùgÄ^¿Ó?RV /¼?-¢üãoz?6ÖÔE4‹h?Bø/Ù?KªŽ"¹?ï‹Zþ_]?‰m"ª…eà?Qg嚮æ~?dT
œì>?ŠübÍL?‡Q ¡ÃÍ?ï[³ÜÌf?ƒLp©ÔÌ?l};Kƒš?_}""ïÇT?™$âõÿw?ç}Có?ïÊp‡nÿ?d°Ÿöy?nÐZ<~s?]†ìm"ðÃ?g¿T'?Uk'=-Š£4FGL J1127.6-4920?ï›wÃc @&Mv«XÀ:^ȋ­À<K€\±±¾@
P_=þ@@6m
J?Â_ý–™4?ÀÚÙÕÉˑ?úZë=Ñç@p
«T­¿å´d@q_>?ïû2¦Ey‡¿ç€"Töοâ¢+¾Ê«Š¿åÃà‡ÿå+OnÓrAGNbcuMRC 1125-490?îȟå{¨¥?šž
d"¤ê?ƒv}—?†¾|Ñ¢ŠH?0Ąÿ_e?–SÍ\¥þX?îìAñŽ‰ý?£#7ýëY?nºô…m?$øYGq?ž c=Œ®J?¡$@°ß(?ìžxdˆL? T…E	?'=¨+ë°?~¹Tëç?ºãËÒÐÂÇ?œ³ÛôEb'?îº8_3ý?ŒúøÒâ#(?˜=¹Þ‹Ï?'é'_ùè³?¢UŠÇ3\?'»o`,ê4FGL J1127.8+3618¿ÓˆAºÏ8@Qƒk¹Œ~(À9m©PÇÀ<!gÝ^ëH@PÚqÐý´@в\Þþ(?¥·ÿʧÑ?¥õØ£‰vP?þ­üwµCC@侬ùrÈ?ë^Ɣ¤gS¿å®É¬†Ü(¿åøq–EQC¿â=fȋõl¿è"‹BhÛ6¿ïÿü¥¬¨AGNfsrq3FGL J1127.8+3618MG2 J112758+3620?ïéyb4½'?`RÒä?•?<þ
˵?6Qú€I?bæÜɉ,?^~A±È.²?ï†4ô|;?‹ElkL?Rmåí­'ì?a;J@?c'?Œ%=Å+??‰+gU¡¦?ï+€>ç>Ê?á«]XÍ?pcÿqÁZ?i+¿>»Ù+?–vøF׶5?~rºA˜ÖŸ?ïÉ
x´§?fÓÛk&UÇ?ió½êZà?[*
%ôm?mÊ0•ýd?\`Ž-Õ84FGL J1128.0+5924¿ïÏVûöl@KU¬îàóËÀ9æ±iÀ<–[žŒG¡@ÎPV"œ@T¤°N?´ŸÈêTó?¶r:@SéG?ÿþÊuÚx@ªÂ»{싿ÒÐǘ°eŽ¿å¤ "ˆÞ`¿ä¤{(߿傚Nʓ¿ï¸Ê·H׿ïÿÿ" 5•AGNfsrq3FGL J1128.0+5921TXS 1125+596?ïá&ÛW?…p#˜?NÏV]…ˆø?RWnü¯…?g=AÃFÃ?"næM¤¬?ïi݂Òyß?˜ÓARH?Vû'¤gΈ?m4£ž?'T–‹jGZ?–Ž²¨òÝ?ï"N‰CÒÇ?ÃÏËÀ®¨?sº˜0©)9?hßoW#¹"?–LjË[\À?HºŠ"è?Ih<(?jLß@z*?p0{%†Ÿ?_	þ3n[?qz½&[L'?a¡Õ~jÔ`4FGL J1128.8+3757?ïWŸ·üí7@Qd~¡ÆÀ9ψ*ÜLÀ<	óˆù8f@ÂQ} <6@?f"‹?¼ÚeÐÝ©?¼Fí¥4'i@£ÂÀ®@½Œ¾)q?©×•	'ú¿×®sûû8›¿åì§]§{¿á'Á(SÜ ¿ê²œÕŽ<n¿ã_gÍAGNbll3FGL J1129.0+3758NVSS J112903+375655?ë½¾"b×?°˜Xeg›?¦"ðP9.?š<Y×+#3?¶Ï–ÄÏv*?«;·Ù™fd?ëo]W§­'?¼§9µ1(+?®QÒÔ9n?²uoY[?µzìYXz?°î|ÝIë?èåüäiÚZ?«CËñî?®Õx\{?—ÞžË*~?IJ®JwÓ?¥=ŠP!¸?äeàÑ?ªÉ"šh€?ÉïŽ<» Q?«rº7*œ?Äxñ"ìi?¡9Ê\UÐ4FGL J1129.1+3703¿Þއ¨^,@Q€Ÿ¸fäÀ:<‹FðYÀ<`'o@á'C'¥.@ðäFfß?¿*^x[[p?´1 ‰Š?ö¾aßîé@"§×Êת¿ï ˆ!ö?âCbn_.¿ä›ª€qªg¿Þ³æ¡à¿æÔÎùÍ·¿çÁšÕü4AGNbll3FGL J1129.0+3705CRATES J112916+370317?ïàÛx-ªJ?b"dJâ?:Ð.š¡Í?1½«ÍÔAÞ?kʁÿz½?a^yø EŽ?ï¢('³ïì?‡W»kœì?H^¬ïä?VŸùŸ³0?…ïùx5½?†²AØÈ?ï6·ßéˆ#?}6ñ™¶µÑ?fƒQ
s ?P—­‡Ëè?–X™á€‡¦?zíÍ!Õ-@?ïu6Ř
â?s¸Ï¨p<?rCYG?[UÜÃqx]?‰íY€ò?qÕex³4FGL J1129.2-1014¿ÔâÚÓÿ#À@GÑn¬†hÀ;9ÌýpÀ<¬Ök±ÿÂ@âŒXhvâ?ý²—a°õ?×5E2E?ÊQÈà5j?ò=0ýÎÍX@ÍîµÕº\¿ïâЯ°\T?ïgÂâ=Lg?éííÿL{Ú¿ÓVŒúk¿æ'4JŠgÍ¿ë#à¯Ø @AGNbcuNVSS J112912-101349?ïZÿÕ¿Ÿ¯?‹>YuÒ
¨?aµû¿‡Hm?WòíŠ{–?'iEÐ!
?Š++`§)?ïCå‹}Ø|?•Ã^à4?\ñýÔúÓ?mäî©yùN?•´.³Á?"V®†l6?íËizlž1?"Ð>^?'ªb½Í}k?tÈb'¹š?®žÏ©Â½?'…øs~"ø?î×lŒä'?×—98?v3R™l‹?s©'PZø!?Ÿ!ŽÖ2Ä?ÍµÞã4FGL J1129.2-0529¿´Ô!J•‰ñ@IçiüóÜÀ9¢š4Ê(À<$Sœ_G@;°É6@ÆX>…w?¶¦¢@²!Ñ?½2XíW\@sbb˧3@c¯˜	?ïzÇw"¿èhǍè¿ç"F{åS¬¿çhÁ?O÷¿ïÿülò¿ï³½œ®!AGNbcu2FGL J1129.0-0532NVSS J112914-052856?ïÝBœñ)Ž?zû,Áܹ‹?`U®vû£?yˆÛé\4?bgµ	_v?\û­ªH
p?î÷§"€ï?œgޗeük?rœÿñ~©ó?"Wš'N"–?œg7o?–tޟàd?îècOò›Î?‡l̀sx?~¬Ñ…ò2?v({Ò¯Îò?›Ha /ÿÉ?ƒÔ{0ÞH?í«¼E O?"‰aˆ5˜2?¢ú²ÿ¯2?§ËŽŠ?¢J:h®Ká?…í'ß)'4FGL J1129.5+3034¿çzcªŸP@Qð¼¾aÏÿÀ:¾ƒ""^ŸÀ<•È¥i±@«*"ýM@<§P;¶?Åׄᦣ˜?²Lêi?ë̘"¶ÛÊ@íØ>šð\¿Ý"±ð)É¿ç©¿+¤t¿ä£TY©¿âÅõåÊË¿ëýØ"kdÓ¿ïó ‰ƒœAGNbcu87GB 112657.9+305242?î°z
&´¶?¥'0¨qH?nꜮfJí?{ª{óê?£	µ'®P?£þÎ8ÿ|{?ï"ùê,ç¨?Œä
Y Uý?K9I?[NÛΝêU?
ôcœEÊ?‹"P"Ä{?î͞)ˆ¼Œ?‰ý#hïó?tP—n¡ß£?jHq'‹8É? œ
yŸûP?†ïaɹo?ïB¢ÑGþ?|®Y;æ ?v—¿§?aCœÒ?''օVP_?zá:Úa4FGL J1129.8-1447?Ò¾P³ Ô6@Eє[l7aÀ9qÈÉ2
™À<ë˜iî±@,ZÝFA®@<bÿ©˜ë?²ýáÛ¹¥?ºWA°N'Þ@ƒ¶æ±za@
'õèO	¿Øƒ´?3°¿æ'Ž¿éŠ¼‡k ¿é+'Ëöä¿îC+κ㖿ï°ÿ|L¹AGNfsrq3FGL J1129.9-1446PKS 1127-14?ïØ೩!í?sÈèûêÀ?J˜R‡Ò?E͓éë¥?p<–A(~?rcКäSþ?ï
Á>Ó?'Ò;àb"C?BÒry°,b?Wf›8t)?‡(H^?'ö1MבØ?ïTÇ8"?ƒ"Wqì¾±?v˜˜Jã?e® d±®?™O_¹4Ô?€öžV´Vê?ïòØëâ~?H'—îíØ?5–<š«?*[6UÂ-G?Tè™XE?E3L÷c4FGL J1129.8-4217¿Ð4r•k.@2˜ú7iÀ:Ç—×øzÀ<¯¦âWx@Å°ù³@"`št‹?ÉGHÿMR™?á|â(ԋ@öOv_Ù@'·þ¯¿î l¼Á¼Î?îPz×6³¿Ù·]d_%*¿ãä±i¿ð¿ïpêÄ.™AGNbll3FGL J1129.4-4215LEDA 566417?劲ƒº>ë?ȱpÁ?Ѻ;¹Àã¼?ÈÉ㙺Ò?©'ùöTóo?±SI(²t?çZBÇÖcÂ?ËŠ'•Í·?Åe¤øB±ð?ÆÞÉÿ\D1?ºbŸÐÇ~?²a2®Q¶ ?ØË€äÂ>?µ'ÚæèJ?ßñ¸-yk?¶Œ`®……ð?½¯·Z? (Ò *?èÆEz³Ç?¦úG2·R?Ã03@öÝa?¤䛩Å×?³nçR<§
?"lf¿'¢Ú4FGL J1130.5-7801¿ïXØy(_ñÀ/¨'ÿ'À9ÿ_,¶ApÀ<…I€|'@!Gø%ÁÃ?öŒ©[®|€?¾ ﹶÅy?ÅÀµ§Â&V@	‹)CÆ(n@RҵſÈp¬æR"Ý¿ïÿíáoq'?ïÿo¾ÁÇ¿˜ìû7昝¿Õ‰ yݒ¿ØÈ\ûƒ™}AGNbll3FGL J1130.7-7800SUMSS J113032-780105?Ł"ï?¡÷öAô¼"?"žTNRΣ?…kö;·Ê)?žùÝ(£úÑ?œKñÅ?ï,¢Àêå/?©ä±áÑ&?amÔ*¿)?x³v­¶?˜Iš(?šjÿ9'k?êÀÅ~_m?¥¨Ç‹J?—Ü`¡ñèª?‹¯‰‡(?Â<ÕÈE4?¢þ8Ô& Ó?ê
¶}`«º?²Û\;ޜµ?p@…í÷Œ
?lU¤²ßj8?ÇS!Û
"µ?³«Mæ4FGL J1130.5-3137?葽í@@<+-À;œ%¸÷,óÀ<ÆiH˜ö@#ÌP×H?õ~z#²Œ°?ѓa^j?µ|ã«`–n?Þ¢èB2›@e‹-m?ïךÈÙ"¿ítÎ6/g¿ïù–#?ïïšø>jŸ¿Ü®_¤U_¿=aƼàAGNbllNVSS J113046-313805?ïp±eû¡?'£«U:0??ïkÙ3|½?9Ì£bD?'~#Û½Ï?'mՒÐÝ?ï¤LÄÙ_?§'äGªX?a‡FŸ<o?wbÐÒäG?:"}Q"?¦4x-FšÛ?ìóÍÁÖ4ö?ŸŠ‡àÇé>?pP¹<,?^õ›û??·\†]Œ•?Ÿ"›‹ñ~?ì«1ñŠâ4?­tß^¼|ª?|ˆÔòäGŒ?‡-4ÆX?¸Ýã$z©ß?¬mýˆµ4FGL J1130.8+1016?éôBö'l´@P'»ƒÏ,ùÀ:e$Ã-çšÀ<b(Cëè@áðusu@Ëeè'?ÀÏa<0?¨?ž)\?âùâå=@s¦¸»ó·¿¾Ä(cvq÷¿çË@Fìù¿é%ØÝv¿èO‡A¨@ü¿ïâöý»'¿å§/^½O¬AGNbll3FGL J1132.8+10152MASS J11303636+1018245?ïA0?ÿñÛ?M4p 
?‡/'W³ƒ!?…á0uã@È?ˆ"]¨PÖ?ƒo°;ÿ`?îïÕXf?›ŒŒ°J?sh¯¨(†‡?t{¼m—¢?+1r*Ñu?—QóÀ4"Æ?í^àVï¥?•°üWß?'ü,W`?ƒå2»Á´?°IÚ¼
?¤Ù|È8?îJ™Ý&	?n3Ãl%H?œôïh¨ýR?ŠœÓ9M¨?™·ÔôòAà?l¯¯N»Ü4FGL J1131.0+3815?­¶Æŧ@@Qtw—|À9/ͶígÀ;Û£ûkq@‹D¤bË@d[Ëر?¬yð±ÙVs?ļ3b(¤@Š.Ýc@6c¿B ?íWZYè©¢¿äX·¼šO¢¿ç?³ÖhW¿è܀žöѿꦭj0ö¿ïÿî' ÇAGNfsrq3FGL J1131.4+3819B2 1128+38?ïNÜ	Ç?'œza¾Ù?'4dpœ?>¨¾v`_?oƒtÕÝlÝ?já«	íŲ?îƒ}<ð/W?¯Ò2a)&ë?†'ƒ:³?¦Sõ!ÿx?¢>Ko®"þ?¢®KãÇœ?ìù™‡¢tË?£ñ*'ԖÈ?¤Œ^õ×^?˜š̛h?«ÚçâÛë?›s¾PÛÏ?ì5àä4'?¡"ªãÄ¥G?°]Ìë	¯?š"ã7Ë*a?«æd»©XÍ?—(]§×Úq4FGL J1131.1-0944¿âˆºÂ;×Ð@H(A*2À:Ò
¨y0À<‹Cp˜@ ;øå¯r@"÷…zÿ?½µj/ž©#¿¨0€Á"Ö?î*käT¨Ï@u<Z#?ïϤMQÂj¿èZԂ"Úv¿â7}DÏ=¿àeòmpEã¿Ù˜,F¯çº¿Öç`Ÿý·AGNbcu1RXS J113104.6-094353?îçc4¼‹?'jóÛ?ll͓¿h?[Ú)ÏØ=?Ÿ†æðŒ?'eFgÇT?×ûËñ? £' û}¤?g?þ¤£e­?q;wŠg?£r²•ù
?Ÿ•?‹Mb?íõŠ
YŸ€?'¢e"S|=?x(æã©Ú?d,2›vw9?­¢B}ðåu?d=ß¾^*?ìYÉ
|֚?™kl›½†k?‰óYŠ"?y&+"*º?¹óLbÕg¸?™êÉWêí4FGL J1131.4+5809¿íϘ4¥à5@Kú¦">jÀ:}mÿ·Û¤À<²bÒ]/†@P1ÏZñ"@M••_?¼´È?œœà²'?âa…V¶K@þ•dU¿û¿ïqsªò‡q?ïõµú"pm¿æÇ1¢a‡¿ÑT‹<߄_¿ãí©¼&Œ¿ä½öp4E'AGNbll3FGL J1131.1+58101RXS J113117.8+580911?ïè"²Æ?]1€ÑÔ¬ü?Aß®r"-?7Ó4<*?cpfð˜K?Z¨Íxm¡ç?ï'í'¤ct?ˆ'XsÀ"?MuÉPÛ=?Z.20Y$Ÿ?‰mYÙrÚ?†¯¢Èl!?ï
Hëìè?€åÉ´«?gèg¤o·y?RGÈÊëŸÓ?›¹ÕïL?~qÒ"A
?ï F€†~?s²"Ÿ§Sv?yïqŽ
Šb?dâp~В"?ƒ@5˜×šò?mZÛ¹L¿4FGL J1131.4-0504?×"ãøô"@J9Wÿ›V2À:¡›Æš"À<H­œ…Ý$@ˆsü|@¶ð<=ð?Ê-ë˕•(?ãØYÞBÀð@cì‰*¶@	ùBWC¿ìŒòãÕ¨?áœ#íEY¿æòŠêÕ¿êw»ûS¿è«ïxÉ??Æ­°½L§#AGNbcu3FGL J1131.9-0503PKS 1128-047?å~Z8‹.Å?ÈŽ¸ä¦8?Ò̌ñ½ë?Ç­EÄØ19?¡µôé]»¡?jMâJ
?ß0©°ôæ?ћý6_Þ?ØNâ¤_?Ñrkn¨-)?Áèj©X?µò… Á?äy0?²ŒÍœWÛi?˓7F´È½?°c9¡ºM?Ä&äHŠ¾é?¥1Ðú1Ú?Ýÿ"gz–°?¸U)^…·?ÚXÞ<Ÿ§?¼X<Ù²mæ?¾¡¢é#&¦?«Gúý'ˆÞ4FGL J1132.2-4736?î+"¯ÔÞ@*R¥'ÛçóÀ:&vŠ ØRÀ<K½¹3'Õ@ üSøû?ÿÌð©Jç…?µc+Ì¿J5ÖD¨x?–Ló½kI¿@"NÀ,€g?ïÿò(¦è7¿æ{B`Í 1¿ÞžáIå¿Þˆ£Ós¿ã3ªò‡qy¿ßÝ~ ÄÜAGNbcu3FGL J1132.0-4736SUMSS J113209-473856?ïªÛ­DÜ«?†:Vº?EÔÞï‹y?B˜ùù*ë?ƒëÆ͙Ü$?…Z2l¬Ê?îmèJ'?°À֒_÷*?Vâý¹ÊÙ?iUo.­]¯?¨jk6/À?°ˆÐ\gW?í±½dß?š]¿Ã{. ?'FŸo¢Çõ?pˆ«Ç$=6?µ.>" €?˜¹¤·•€,?îw»^j?ˆëfYøïS?ƒ³
ŠÜœf?jéØМ^²?©Ë¡'òK?†íO(Ç[ó4FGL J1132.7+0034?íזr{P6@Lµb8Ú<!À8j¬=áÀ;ÎpmP@–Eý`@åM|Š•?ž±ç÷©"?™­ƒþŸ$??÷¹÷2ú(@	á þ'bÅ¿Ñ:b|vóý¿áX»]c³Y¿â¨B(ïb¿àíàBËV«¿ãÜU•:¿æµ£ñpwAGNbll3FGL J1132.7+0034PKS B1130+008?ïÉ8,À¤?p¹î'eCÆ?=©l]Ïþ?6£¶û¤,?y‰RÚ0z?p>ļ?îÉqç¶á•?¦{=lҜÕ?wb#&0Ü?\/ž]ò®? |ÎÀ›?¢¯AÕ%X×?îëÜ|7I?Ž•MgœõÈ?vv`DS†?w™B±rdf?œæØhù$?ŠÑ"Ú‰9È?ï‡ç†U­?‡M½yZ?ŠDLN~¶?~æ5ìŸF©?Ž¹Ïì*?y3N{‡Þ4FGL J1133.8-2048¿ïòIÔ4u(@CA3 @|ÈÀ;J¥»æË|À<¬.î*§@ #áÜ~q?묔é0°¢?ä#²VÿÁ?í'I†\@¥#±µð?úÚ!nºË¿ë<…ÂL@?ïèq£±J¿æ­—}_§?ËHvü¶Ÿd¿çù_!£"ÿïúDÕ&§AGNbllNVSS J113350-204852?ï¶,g›¢?–PU²?'³Þ½¾o?~Û.$ËÙ4?"/²­¬?"ûè;?ì/òÌ6t?ÀhöÐ={˜?¦ë©ö?µÅœÇA™?³/•QO?²+Z‹‹·Z?ëü4°}c?£¹ê?é?›fh2?‹i«ó â?¹DÀXϚ¶? À¦"§†%?èŽ([3Ž?¼qDoÛü?™ŒÃÎ-?¨Qæ³âՀ?ʕÆ3™p?»J`aN¬J4FGL J1134.8-1729¿Âùéæě@DÔ€À;Wc$'†À<¢Y …F%@" Ӊ)‰ç?ôÁjî‹?ä),~ä®?ӂݕqì¬?üýî'ð2-?úkQ'n×ú¿ïƒŸâˆö´¿ëÓÂõ³uä?ïúgïÓb¿åfc á¡ñ?¬Dà"º^¿ÛUü wnÌAGNbll1RXS J113443.6-172853?í!&©
 ?±W}É©ˆ?oïL¬]?r7«ù=Ä?²‡~ RL?°Ü°×ØÔÌ?îfÿUo?©rklBÒð?rê)MPÝ?"sΩ?§\²ÅdÑ?§8>Ûô?êøψª?©'\5ü'?—LÔÞ?‡soë…ÀN?Á6_@'?§Ü'¬úx¸?é©ç·f`<?³iulà…€?Fù½MµM?W1éK¶ç?ÉAgeH1[?³]3Þ]Õ4FGL J1135.1+3014¿ïþSmwí@R@I<‰ô
À:ŒNrSÚsÀ<^6=@IϚ¦ã@ôQƜ1$?¿7)!Œlµ?†æՕ%õ?ËoY­€@_²ïyu?¼˜-žHÕÝ¿ä©Xž§ m¿æü­e(¿ß¦+xSδ¿àï€ô‡&¿ïø
ÞpAGNbllCRATES J113514+301001?ïÃ^wpà=?ƒq¨slޚ?C"-é³6×?9ݍsŸs?{à>ŠY{?ƒª}FÎû?︭åo1?'ôsË6Dú?:tCÝ×u¼?NÒY+ét?çµw¶?ôèò%?î÷À[©kÂ?ŽíKÆÉ?fN¾,â'ö?Y™†­PQ?ž>Å65Ÿ?Ž¤ïÉF¤'?ïÁõõ‡r?bæÅy.íq?SòmS×å?A‰2säXH?zjFMR?a²@sÉgÍ4FGL J1135.7-0427?ï–Ã`E@JÀI¡3ÁÎÀ:Júì.'À<'cXK@4¥šõÿ@´£@ˆÊ?Êóˆù8e¢?ւc€Wÿ@<»r1v@p8²N¿âÉäà"Õ»¿ã²['ÕÝ¿çéüÞbvm¿êTÅ¿'Q§¿ß^?cR¿ïÿ‹Á>ÏAGNfsrqPMN J1135-0428?�â"*?wä°´öÒ?h¯P§·¯?g¤_ÁÒO¬?sÉfª²?nÊgˆÑÃ?î bÐ`£?£k=ÔqÂ?{ InKR?‰"Ê -¼?¢•ÉÌ,e9? ·)øÓ¢?êQókª­X?¦'}{…?¨ÎpE±9?'üGìz†¨?À"–OÃÞN?¢Èúݦ?íœ7'ŽG]?•MgX&á"?Ž
 3½íû?{ö|h¡…W?®¹þÚ,»?"Ò:‹dߐ4FGL J1136.0-6824?çU;ù!áÊÀ3wÀ*ýÛÀ9ßzR÷À;Ý=ïí™@À¤[>•@7Á•aü?ÁÜæujeO?Æ9,œk@þ|Tå5@;BÄÕ?ïó˜H`Áâ¿Ð'¿ŒÈP¿åú!ßxËï¿èûYbFò¿Úa3ÁÎl	¿ðAGNbcu3FGL J1136.6-6826PKS 1133-681?ç)ÐêCEH?¼«Þõæ\³?¬šI)söM?¤^-k?Ì2*•íM?ºfMÈLá7?Üý§Ž–í?ÉS[&²?˜'1®§Ã? (af+×â?ཫ?~Ë?É;¥…?ä—Ólj2?°:¸£j?°Êp'z§e?•c'3(™?ҝܴCÃ?¬~u˜E#Ü?æüÉñL½3?£¹ƒoñ6?®
^ú»b?—ÌIÌìx?Ìi£\^?¢Bø4…N³4FGL J1136.2+3407¿ì˜Ä"Ò–@Rûüe@ÌÀ9犰ȊHÀ<}Mæ<à@¿8Ëùh6@ÝGËÂâ?µs[|T?¾w¾}~°à@.¾`"€@Ó×½k°Ó?ÖùXD¿ä´Ò9ô"¿æ{{*·å¿é%ãõ~z¿ç`…¡j€¿ïÿû}º@AGNfsrq3FGL J1136.4+3405MG2 J113627+3408?ïò58!I?cìB GF?96¯õ'5w?4¯Å¬
<?UGâè\âD?bé‰òM¿Ñ?ï©Eœ‰ç?‡ ÖU÷Z!?Bî¯Dâ}?RÁxbF™?"ÏdeŽ?†zÇ-ëB?ï)n¿0´x?€¥uw;#'?nö¢X
ÀF?_[kIŐ?–óSÎç¸Ü?~¾¹¨1•?ïæW_TÖ?TãÛõ}??Qxúf%ߛ?A`_ڔÊ}?`ì#x?PéRùlÕf4FGL J1136.3-0501?ì4¯ÙÄM@J‰¡ÎòAÀ:…0íÕ·À<³çcQ@Íe+'öê@º=c7ݽ?і]çM?Ýî~ƒÄ~@r+EþçÒ@'rÒZ€?ã'ZS<=¿âқ®FÏÈ¿æ̀÷Œ>¿é¦zÞB•ý¿ïÿÝe¡D‰?ïþXËs0yAGNbcuNVSS J113607-050156?èÝ|°?À:ê@ŸÛí?ÀT?Žd¦J?µÜÂKÅ´?¸nø*ÚÍé?²˜xMe¹u?âÌVi%x?Ïl÷A)'?ѐ¶ü_Š?Î×YŠŸ'7?Á­;'b«?µ"ù¢	ë¹?ãÿáv?°®üº	?Á\:3'-?¡MáRæ??Îû§zF–ø?ªŸ/SøÎ?Þ'zà!?´]
ÿõ¸?Ïû>æ#é?´#Š0Ž<?Ñþáu'
ê?°•áWÁI54FGL J1136.4+6736?­p]úmU@Gú">iƒÀ9ÊÛ-¸ŸïÀ<Td«{Cm@ o@)»»?ûB%YUÜ«?¯bJßž? –´6þÄÂ?óišÐ@
"M'ëð?îŇ^-³?ÉO[¹¢¿áµR\Ä&¿Ô.ÁÙ©ª¿Ø1tí¿Ù«¨$v×ÎAGNbll3FGL J1136.6+6736RX J1136.5+6737?ïÌ¢ÍÈbz?iõ‰_H?Aˆ÷厳a?4Ó#ïÉþ5?w}zí
?gìw¿ ±²?ï›r·œ
Y?‡ƒJ±}·?GÝXàM,?V€ˆ!qÆ?‡³4Cn¥&?…úõ<˜v?‡å™?"±¡"C‰3?f/õ3lŽµ?`Xd,ãÊ?ñ(•ºõ?ƒsè×rãý?ï>ª¹D?z‰4&»ç?rÂ¥€€¤?]%Jm;nÔ?"zHÝ×j?w´Âýûü4FGL J1136.4+7009?ïùi$©$@FÒ·`,'À9¿¤EÀ<	?öå@x{‡µÁm?üÕýb–Î
?¢cŽ"u©X?yÁ"KùÕ?؛Øc-÷µ@
Ãsٖ‰Å?¤A_r>¿ØªÀ2Š—¿ÝžN¿Öš+¿Ù¦_$Ӟù¿à=At>–>¿ÁÃõãœrAGNbll3FGL J1136.6+7009Mkn 180?ïñ(¼!?bo>s?#‰"g¢F?!Ár\)^.?[h}úðÈ?a‡´lB
?ï"ëuy·½?ˆ6ÑC®U?I›òéa³ú?[†9899f?‰+crûôë?†fËÂpF?ïÝÔ£ÄU?…·•¦`ë?hy<+.¾[?b=(¿Äv-?šµæ!'?"|ÄB»¹ë?ïš3£?qó™÷Ü­/?dn
£ Š?THœ?"^4°–îÂ?nR!Áå74FGL J1136.8+2550?ë é±¬WY@RQõ@‰]À:¯Q=à5_À<–/#ÙùÜ@ ;%Öÿ*Ã?ÿÇP ©Ã³?ºf¨UŸß¿£Ù,"=Š?êTø³¥@oZN€?ïôÜJ婭
å¿×Fb$S¿ã)ªžNµ¿Ü­ž^Ok£¿±!`ÍË$AGNbll3FGL J1136.9+2551RX J1136.8+2551?†§i2?€B˜"âøN?X
"Ê֖?O°çF¶??…"]ÌX?~ê ç¹wº?ïiöj#ÌÞ?'€†pp¿?OVWòaE—?Wæoˆµ¥þ?'ÆûóZ?'Ð\פU?î"ßvªÍÇ?-1²t¥?wsh
ª?fÐæc6ÏÇ?ªã–¨QÎK?GÝ`,Œ³?î€?)d?ŒŠ¬°ùœÈ?€×ïÊ?pÙ™üµ)?£õ	8=Ìl?ŠóT]69}4FGL J1136.8-7413¿êgv±¸À(4¹#¢œxÀ9zŠ‡¿À;ã5ÍAfÓ@Äù·;–@%Қl'q?³z&P Õ?ÊËí>\\!@=s!_Ì@‹ú¶j	ß?ïýaŠ^"3¿Þ
üGä› ¿ã4ýØ"¿æ¦ãÏGÑP¿î:ò¥µ1¿ÑÇÒÝ2¸AGNbcu3FGL J1136.1-7411PKS 1133-739?ÁËǽØ­?³ÔðfÚ¢ä?àX}' 6>?Æ"¿ˆMš?Öi þ2§-?Ãxg'c€w?Îÿê7øSÖ?ÆÓhƒ\?âÛ4ꁰ²?Ë{lž,À6?œBéa?¿<¶ë«?ׅžwtÞ¿?²{Ä
ÿ¸?×o+…9tq?³*gd(\"?Ñ6Q¬Ð?ªÐÓ4vÅâ?Ðï[ÄWÒ2?£p[r¢?×^M¾Ïœ?¯^\ôÐ?ײ"íé^2?©§5?j—4FGL J1137.9-1708¿è²ÏUh<T@E"_ !¸À:–,Y$^"À<CõwæÁk@ ìç¢fé?õÂFçE?È(éè‹Ð?Ñs}\º@	£qÚ7ï[@)£šyhw?ÓP¯°\S¾¿ÞDÔÛ¹ú¿Îì%'›{?½e)$'"Í¿â6o]…í¿Ô?·¥ôïAGNbllNVSS J113755-171031?î"#Õö?£ådÌû;C?è³Í°ð»?{bt4hko?©dz
Vd\?¡çŸÄªšË?ï<3]XÉø?"1ËΜÜ?X1§'d7n?`ú4{)êh?–öyâp}‰?'wñÜÉ?ìR˜–'p?¡j¬úr{…?˜ÆÁ¿V©6?ŠOU¨Îz	?¸ÛºËuÊ6?üGñ 3«?ëBà\+$Ö?§üšR1Ç"?y F'¨¢¢?n	«…SYœ?Â+|Z¾'‹?¨ïñA¤&4FGL J1138.2+4115¿°*ÖVÒÝ@QXŠï²ªãÀ;`OËð.À<±§ðtqÂ@ 4C(ž¯®@,ZÑÝ®?½F‰§357¿¶dù(öC?û{
¢ò)@ÚD…ëçÅ?ëçlU"°L¿èùŠ—ž¿ãù.ŠWw¿åÛWª¿×ÙôhI¿Ý¯çä«:×AGNbll1FGL J1138.0+4109NVSS J113812+411353?Ia¹Þ?žˆ¤S™Û&?m_;˜O	´?_œ°ù~£?¥ñW°_q…?øіXv ?îú~Íþ}6?žö¼cý¦?d—m+­s?tËþ^6KQ?ž8šÍ#o?œæöFt‹Ç?íéÿ•ðI?'3*×ÆÈ1?x¦]=†L?dïÂÈ?"?®KNÚùJµ?ÜÖ«b‰?í'Ú!Ÿj? ¯ö«e_‡?‡æ}µ¾?€™Ë¦O'?³ÄlãQ ¹? ´GÊíÆ^4FGL J1138.4+4857?ïÁG·¾a"@P†­-ËÀ:¬¸ô¨´À<¤k'QÕ@€šˆÕ@ÛçòÛ?Ào\¯-€¿¢3NSÙØ?áz‰hÉíõ?üâf´êØÑ¿ÙÚW¤×J¿ì`¯7¿Û¨üct¿ìåvã)Û¿ï÷³•Ä"?™A_(…AGNfsrq3FGL J1138.2+4905GB6 J1138+4858?ïÈkšÝ?{';ýàB<?myïN!?q¼¢g¿Â?jiȏuÔ÷?qiû·|…å?îWÈ{z?¥²>K&?m¯ôHÄô? t­ "C?¦2Ç{<'(?¡Gçn˜«ò?ìÂ÷3ðù?™¸M¼%ºƒ?EšÁiñ?A{Â9
?²–ß°$ƒè?"ÖC;úm?î~_©µx?—ä<ÑQü?žÓOOàT?•"±":Y'?'azh?§5˜6ÂË4FGL J1139.0+4033¿ï""HC)@Qzµ^ñýßÀ:C¬­r"rÀ<4cʪ³@eMÌg@ŸžEÐÄ©?Átˆhî?µÚçÜr²?ñ¦+]{Ü@Á¿M2bÔ¿ëv_ß
¿ԕOó]ZN¿èƒ_›q
.¿ê"ö^ìtˆ¿ä˜íÂeÀ¤¿ðAGNbcuCRATES J113903+403303?ïòë÷â?‹¤ò£rJ˜?8'N]æÝ!?n¾RC!
i?T>*n'ý?ƒ÷$¯WSþ?¢åÆ$?‰¯´ðråw?Iµœmןû?_«ÓJö?ˆt½°ýC?ˆ——Zkí?îÏ]ÁF¯?‰qÿ‰5ÄF?|èþšiv¨?w­[W¡î?žÚ8œÌ‹?…†ò)Ü¿?ï–`|¤¢?sDy«"?b£MNŽáã?TS—¢õß?…¿
ƒWžÉ?qÐÓ,±_ 4FGL J1139.0+5530¿Éƒ²D¾Ôo@M_â?$ØýÀ;æéóN@ÖÀ=8C=lr@"ì¢$'–H?óÂ}qDç?Ög†aƒ}£?Î1·ÝýKÆ?öäí@	Û@gÿtißB?í!¼{¿ïÿð`OËð?ïú­EH­?™Ü8{$A¿•↦¿ÙsË©·AGNbllRX J1138.9+5530?îª5<u?´öÑ,ܞo?e:ÛòçãX?`ßÌ¿frï?®a®æýº~?´È™Î:?îæ
 ÓÎ?¤̉\þû?cW=7H&?v« þH? ikŒŸNŠ?¢öóŽùX?ëý˜€?£ HÛ²än?ŠæJ4¦g?qږ²å?½æuÕjp?¢Ú·)Ò?î.7)š?›ÑÝQn (?MÅCô?Jcaåõ­S?¯8»7f?›³xC£
4FGL J1140.5+1528?ì̱8òÕ@Qu'·þ	À:þX;*xzÀ<†[3,}7@"«Hî†?ûŽîDì™?Ç#KŸÐ-?¢8¾Àù
?Ú'Â	Ð8@Õ̉…û,¿èÉN][$ê¿ïm"Ãqx?æ»ss•#¿å·¤ëàŽ¿"Ïюþ`¿ÓÏ-"óoNAGNbll3FGL J1140.4+1529NVSS J114023+152808?îñº8mˆû?™HçkO}[?K'ý²ÁŸ»?E0£LÑ¡x? w¼'\iÞ?˜ýYs…Šd?îè6iHÜç?®]ý+צ?dL­O?zd$ô¦Q? 7ÍBg\˜?­6ð±Wà~?휞ï Äe?•?#H(y?uÉXàoº?d'IºPÑÒ?±ÊÛíkÕÝ?"KÀáo?ì拏Ða?£ºe
s‡?dŠà-ig?e–0‰'­?·Þ'j}É«?£žlË{4FGL J1141.4+6805?êÂI¡3ÁÎ@GÚ.	þ†ƒÀ:NjY¹À<Ž-ë˕•@ ÏU¢Hê«?öd»®²?Ãß\œc"?Ðñdûµ@èDŒ÷ʧ?ûº¤¦½ïd?ïåôñ¯e¿ï²¢´ËNH?Ž±ß¿È¼]¾ÍÖ¿âT,Ý®œ`¿Ïo¬ö˜£%AGNbcu3FGL J1141.2+68051RXS J114118.3+680433?îuËO†?¨"B»./s?˜èÒZä?•¦þ‡N\ª?£d:MÚ#?¡nDY•¨¾?ëÝ0UQ;>?Á	#ˆœ£?¥ðÏD*)ú?·¯Êçt?¶³a
?³…šG…æ ?éNiô\&?«\ϗN€?·º)à2&?£§,§›D­?½Ò‡Q>? û,ì­Ó?拂
o?µˆžcôu8?§Î)v³?¢6Ɨ©˜ý?Ð(&ÊL?¶j	š-i4FGL J1141.5-1408¿ÙÀ«gˆ‹@F°Bž
A¢À:žë¥ÕçÿÀ<w»dg@ y‰®¿ñ?þãM­1üÒ?ÁBÎ[ÃO?¡p¡æð?á±ý2Æ&@
;"ÇOŠ¿ã7a–5¿ã,o_3l>¿Öf9ð¼–¿áòʍWkø¿Ûï½µ'®¿ß¤õî.FAGNbll3FGL J1141.6-1406NVSS J114141-140753?ïÙ±þ)s?fRH䞆?9‰ý¿2 5?0n\×I`?q§‡$ø9?e&z"J§?ï©uÖý?"Ç)Œñ?7weƒ2?H¥0Õ®+?"æ8OP¦ë?"<ÊóJÃä?ï_´J{?€Da-½í?dŸ…Ž­¶ø?]2²œë;?™€ÊÀù|?~
Ò5Ý?ïXà¨¸?v^¸¨ÃBË?LaŽã‰ß¯?9"ÄÜ=Ù?"÷x®™þ?vDqžtw4FGL J1142.0+1548?ëŠv´oçL@Q"¿aª?À9˜€£ÿN)À<7€@,?ú@rŲ|>•@zãËìÓ?®pC£²û?†oHQaÛ?׏ó"
3`@ÅZ»g?קּ'›O¿ß¡D¾uñõ¿å`½§?õ¿áVÄ!Ølé¿ãÌ€ˆ¦'¿äŠšXz"AGNbll3FGL J1142.0+1546MG1 J114208+1547?íÈ»(]ÑM?¦2J¹³Ø?€ÈÝÂÃz?uwŽ<rÐU?¯B2:O?¤óR¬âéL?ï¾DBÅJ?Ÿ?.ÜqÆ?qΗNՏ)?ƒwkÐ"8?š´'£ñòë?š5'/1g?ëÜcPŽVx?¢îìœ?–àñKnj£?"bô^í}B?»d©(±±œ?¡1ɓZ®	?íD—Û½ÎÜ?™9ñÙV¾?©¸¸U= ß?"«$¹é,º?¡ýÉîåñk?†¼(•AV†4FGL J1143.1+6122?²ÀÄkÂUV@Jð² yLÀ:dIÄo0:À<"Ö"Üs3@±Fúæ:²?û͓fy±?Á9r½aÊË?ÐD¾ÂH@=À@ÍOª@xKôL!?ïñ­!5Ú­¿Ø´EíJ¿Ö˜"úUò¿×®«¤‰Ø¿è'I†[Ï4¿êÆ|†c[ðAGNbll3FGL J1143.0+6123GB6 J1143+6122?îìeîâ?¬/k, ñc?–l–Ó?–E|ŽÅÌ[?ˆ®°K¢Y¿?¨F1j%я?ïk$Éáû?'™•¼CÈ?T-Và­@?`ýg'¹˜l?'X¨XÃÜ?{—Uš?é_[ŽêÄ?°¾~ÕB
?ÂO÷P¶kC?­%Rzÿ?°e4ç?O?™ñ…úA'?ïVèç	¬?z°\Taý*?r7<:
?`
iqp?ŸÝûn¿?vÞïĒ¿¼4FGL J1144.9+1937¿ïÿÁ2Ýn@RAÓØZÀ:byz?a?À<Íùóv…@y¬'˜ï%?ÿÑ!%µ¿?º'ú E?~qB"ãÒ?Å6½+o"?û½'(z?ïL¾õsµ¿ã¥óD/Û¿ÒñO‡¿àÒýž%ðU¿ã›šu%¿ÏB7]xêAGNrdg3FGL J1145.1+19353C 264?î³Ë†œ(?¥Ï¬SgÙo?iJB}K]?aq(°šÝ¦?£.¦â«O?¥ZòCÿV­?cŠ'?¡…ìÊi	Y?qõG_ý¶?z:û¦?£ã«k1? ;¢j1¨|?íŠéiLg?"HvÊ÷™?'¹O}Ìö?t ì&QuM?±Q"­ã'?'×m7®H³?ë1èۇ±? ¾ò¨ìõ?¦ææWúó?[˜KF€?»fE°›]?šã×øÔ¥Þ4FGL J1145.5-0340¿ïM{ì	©@K«#c²WÀ;¯ä	)tnÀ<ßæ Zé[@ ½'³K?ùÌ(bÙ?àèä?°8?à'õ|ï>è?ýƒîÑíž?ûîi_jÖ?ë.2x"P¿ïÿò(¦è7?ïÿVW$ª¿Ü^äq¯¿ãü°TDz¿ïÿÀäa>AGNbllRBS 1029?êm<ÿ;\?ÆSÈä')?€¬FÀTw<?"Áðx°ŠU?Å@G—»!?ÆÂ÷ýîA?ì{PÍV—?¹\©£¿Ž?—sLËCˆ*?¡ç}2ž(?¶H¦bI?µHòÏ ò?êÔ=Ñ+M?«blnm?"šæ6Õr?"4Çً»?«úJä?ªUí¥Ž*?æÚú0î~?µáuBî?'VÈæ"Eµ?"#ï=; )?Ñ4Ÿº¿˜?´Å5ђÌ4FGL J1145.5+4423?á_÷·\"@@QèÑQ­À;z8«B9À<ª"á{°{@ÇRÏ۟ù@oÅÀi<?» ¤iT'¿À*Ðù'7}@äpùg@.°',ä?ïŠ[…~¿ærùпãÓõ €"Ž¿ç
:'£¿âŽ7€ŸÍ¿ðAGNfsrq3FGL J1145.8+4425B3 1143+446A?ï¾"¦ë?~\"Ó¶<Í?gêì¼íÙ?b¹î–eØ?u?N¶<?{fV•¦?îù`/Ðqf?ŸÕÃõÙM?oïÞÞ?‹¡
"ß?œÕþE¶H?˜+SeèGQ?í¾5Ä^r?"+Ûf8è?‹o¾­{Õ?~ÿås({?­C¬øryø?â°ÃëË?îÓ©nQ?—g
†¤â?'U ÂúÞ?ˆXõ`'E÷?¥gõ
{?ß–ƒÀß 4FGL J1145.6+5552¿ëÛPPØé@Msb¯È°À;¼±AV¥À=	l«$™@çX"Öĝ@=m;l½˜?Ìþ0­ï?Kèü}ÉjQ?}âkÅuëj@70Ûê÷Û?ïˆ?Õ%¿ß"ä"'ï[¿Ø|Õ¾Ž¿çÀùYó']¿ÊòëÅ`qÛ¿ïÿÿ&¦³AGNbcu87GB 114248.3+560915?ï`¦Ø:48?˜>ÎgnF?iC/M†´?ls@ýÆW?Â¿èE?–BEô¼è?ïô2¨áÈ?™¶3ÓéM?Vq»Øeɝ?f"ÇðÜZ?›:]í]jZ?˜Ô½â't?í7.'‡"?— RøHE†?>¸`f?"]Œ$zè?²žË¸z?"ÖfJg-?ï]ûùû??}y›eޙ?\Ô(«A²£?V4Um"‰l?'s>5äR?|ð"¥œ¯¶4FGL J1145.7+0453?â"'¿}2@Og+©ÑöÀ:ìH£ÝÀ:À<t·×rB=@øW8ò@"{?;2?É\–#û¿³waì?çšr­™@ҘÛпÜބÛš¿é <€¹Îÿä†(¾e*ý¿íѾ¾í9?€ùu2˜?¿ïåﳁ¢,AGNfsrqPKS 1142+052?ïºÄl*A?ƒÈÜîä‹?^ÕQ'(U‰?_š¯VxI=?zèu' Ê7?Í×7ú‰Î?ï†Y¶æK?"iwJðÌ?UÁáMúZ?r¼­óÀo?‹À­h£Ã?Ö|£X&ü?îBßñ=7?"f†-(ˆ:?vŤÃª?skDš,?­#}3ɂ?"w@»fÄk?ïáà,Òà?b®Æ/!†L?7F~֟…?7'
ò?k7ÞL ?aß}i_$4FGL J1145.7-6949¿ÙW ÈJ~À»?l&šÀ9èn"2QŒÀ;Ä]¨QÃA@c6æÆóð@S'ˆ?ŪD'?Ìûúâ´À'@é¨ÛUüŒ@\\¥t?î¶ãâ.V¿çÜ¢˜E܃¿è›¬>ÿ=¿î$Ä:Wã¿Û7ã¼R,¿ïñâ0`†AGNfsrqPKS 1143-696?ï(R¤Î¹^?¢é®Š»?_IÆ¡dyõ?`ž–ëN¿(?™üŒ©?¢ŸÄ+—É5?äz-ë¢D	?ËR›lÉÞ¾?ƒgš@'?'ÔOX0?ÖpgTÁwÅ?ÊÖÎÞÖ¯?ê–R×¯%?¦<0kH=£?œ"˜"+–;?‹hUT"\?ÂB®;У?¢ãÍæ_Ž0?ëhÛÃâP…?ŸY7ûxEã?Óó­{zk?~⦡ÁŽŠ?ÀQµŸD?ž¡qh°J4FGL J1146.4-3327?ˊ@~RôÍ@;zãâ"À:æÄ©Ü¡À<€ëaŠR@26ï©@íàBËV«?Ïڿԗ?ÒmõJ‰;@;ç+y+?õÑÊWÒyà?ïõ/¢/k?´€îýÏ#>¿åÞ¾Ò8F˜¿äè)UJµ¿ïñp»Sþ…¿ïÿÿ)@k*AGNbcuPKS 1143-331?íúEp×Hb?¦tGˆD ‹?‹å¥BX?Ž"‹´•?©bcÉ:ôO?£'+~@} ?㏞׳é?ÉT:qè£Ý?ÎW4n:Ô?È}«y¸m?ÃjP5'õ‡?´ƒ"43?èÊK%¬i?¨‰YƐß?´»2ÃMüL?š`ñ=ÜèJ?Ây:¨Œ4?¢6û_›k?ÜU‡8³>Ï?®êOÍ?ÁA?Õ)FEè?³QÞì"ÿ}?ÍdpxŽ?¦G&oYÈ4FGL J1146.6-2902¿íÄiÀ@?¹Áç–|¯À:ãòènÀ<Œ°"‡áá@_ʇù@<'Éä»?̟á²7Q?ь!f,/@부#§@†)ç0'?ä1£{š«?îúÁ'›ü¿ålÉVö†Ú¿è´Zåÿ¤¿á˜'Bdÿ¿ïûM³çùyAGNfsrqPKS 1143-287?ì½ö";?¬8ïhêst?¢55LUí?"âm†?°ý]¥30¡?¦YƑE‰Ž?ítîÖr?±Øû¾Úõ4?•*3Ɋ÷|?¦-;pÍ7?®)mM?§!Š¯÷`?ë32­?£_Ú¥œ'?©bgëE??"O8ˆá?¹µâz(N?›L™p›?ësOòB8?¡{›£XÙ?¬Åá¿(×?šcHÓÅïÕ?¶}qÒ?•ÛèøŒœ©4FGL J1146.9+3958¿'ß«ÎYÒ @QÝ÷'j@À7À¼O§@À;ŸÝkí@ådÉ-[@"ÚZT	m?"Mé=Ï?±/à~–š@ɝæ?@ZĨ»ö¿³ÊÅáv'$¿âáT¾É(þ¿æHmWoÈ¿å'pjÌ&µ¿ç½jΪó¿éÌò!+ûAGNfsrq3FGL J1146.8+3958S4 1144+40?ï 3''Κ?"qø n³Y?QrG}9®?QkS b´?…Äޖ\²Z?ƒR †Ž¢"?ï9Ät%Qª?éÑ·‰O>?bïE»œd?tì៬?–iˆÃâ:l?›µiÄó?ïU*—(
X?"¤ó´×÷e?rtAHñk?pÜP¶"í'?Ô
¬–?®t¥îv?ïó
i?M_ ]¾?@š¿Jìń?7\¿t6?Qž+·c?Gö{Ží¡i4FGL J1147.0-3812?ïA®fkÊ@6ô	å\ËÀ8v`' ×À;±d¾ÆyÌ@là{U`Û@G
=p£×? Î»do–;?«ð~ã"õ@.®@ð‹@½áÓo(W¿Å*F$§5¿àÙ§'æø¿ä‰¤úì/¿àõo]°à2¿è¬übf§¿àÍ7¡AGNbll3FGL J1147.0-3811PKS 1144-379?ï䅚èÅG?b»iϚÞã?6ÏP¹A™
?:ÁO">ç·?h {…°?a"EÖ|C?ïw¬u_¢œ?Ld?Wáà²ø˜U?iZyK]ož?¦'¸F\?£"ÄB;?ï"¶qó!í?"32™1Ñ?t7lÝ%š'?q7J,eÞ{?–›VŠR[´?€Ö:ónù?ïÁã9Öë?fwS"±c?\e,ö?LÛ)%üö
?x%Ã%Ž$?cèCÞ64FGL J1147.2-2627¿íØ2"œ@A\1YÀ:
'@ßÄ À<T·«c@2—"@÷$œ—zÛ?¼]v}µ¸^?»´jÀ¾ ¸?ù]RV)Ž@ìéõýr²¿à'#€Õ¦¿ã{V'Ô?¿èÆB¤À>I¿å'EØQeM¿ëۙN?F¿ïíœtÜAGNbcuPMN J1147-2625?î¤|L<€?ÄX'‡¿v?‹Xw—jP?¦騥†{?§OšUzÝd?¿¶††[[?ïªÂ÷ºRV?ƒOø°'É?A'Æ*Ç4ž?Q±÷¦µýÏ?"<Å®¾÷(?'MÜ3›?ï45–Rê?}µ	ù+9ð?prèùþ?bey³"õí?•\¤Nõ'©?yÇf6.	?ï¼­E/žf?e¹¾!ÚÛü?\Þ%\_ì»?F?Џ,ìÄ?zqÔÑò?c+2Î4FGL J1147.4-6758¿·þu$§üŸÀhaýKÚÀ:I:MÙ§§À;Ë
ù½Ç@_‹p¶÷M@§ø-ýi?Ì@x@-˜?ٿώH,¿@žÈ~‰rÛ@uœ9\¿Ùçwþ"E¿ãRôÏJU¿åD(Müã¿ê­x:¤A¿ïþûž‰s¿ãlqãr*ÀAGNfsrqPKS 1145-676?Ìóf®'0û?º†7?Ë%"ÇE'?¼í¹90ò?áùÝÔ-¢a?ÁåRwúÝ?Æ«]FÓE?À¶X"?¸lP%À\.?¸e×Ìî?çGž©Ã©?ÃH˜®Ê/?ÒÀúÁ'€?ªÌ`ë!v#?ÐÌ«½)¸ó?¬JXîÍ*?ÜsCHČ?®ìeK`»?Ëþ›' ­]?¤¾	ÕJÖé?ÌõcÈ×L·?°°vpÜÉ?áÃ-B{?³:kεp¬4FGL J1147.8-0724?ï'L£œ§Á@JßeUÅÀ9yæ'æÀ<TTëêŸ@d"ZD[@¯¸õs~?±òù²3†?Åä=;IØ@Ø\$ħ@~¹*³?ïÚua«ì'¿Ùº·Á¢Í¿çêßÂrÖ·¿ç_XŠÛµ¿æ…Lp¿ïõæÁÀ7AGNfsrq3FGL J1147.8-0725PKS 1145-071?ïàÛUF?h<í糛?W†"àɊ?TâÁ‹«å?ca­vEó ?a¤Výk›?ï‹Þ[ìU?… êi•óÉ?OûÖÓ?\+PE`¸~?‹«—¸Í$?"-%(V?îTÑrÁ?"q›¯»?ŽÝº¹8?ƒàNo¨?¢û€0Œ*?‹ôO@Á· ?ï­=îÑßy?kÖn<'Æ?iÍōVH"?YŒ"nòÛ?|z%Ðe¾?eׇ¶«ô4FGL J1148.5+2629¿Á0øùÙþÂ@RýàŠï²«À:–°ä+ŽÀ<oÅµW@£I.G;(@§±9ÉOj?ɞ¥2?¼HÛæñN?îõù`½°@¹î£·*¿ÛBž54À¿æ;T»,¿ëSà4éí¿èvk—'ÏR¿ïÿ³©æ÷¿ïÿè+ÍäAGNfsrqTXS 1145+268?ïõæjtäÉ?Sí5$¤Q?FSŽ4—,?FËw Š?B`ž8Gv?MS
Ñk¬?®ßûÁ?ˆže†Ý?NîíwG#?b9PôÒ0å?ˆ©%v	›?†'(\È_?îà7AqgË?"òD\åTÈ?søÃ"ÉÎ?dÚQfÐ?Ÿ2™¡
TE?ƒH€r´+Ö?ï½[¤4
?gSáÕÈ</?f,F…a<?T¥aÓ=W?vJ»J}?bñÚh!ώ4FGL J1148.6+1841?ؕRÓó˜Ð@RQ'U°5½À:œ2ƒ
À<'HÌ!¬"@ÚÏE"@7›x¦?Äuƒ9ÛÃá?§e"ÏãÙ?ãO؅g³n@Æð)s@ê?ìô´!Û¿ê&$V÷]š¿ãÃQùÇכ¿×$:ýöe¿é Ÿ>À¿ï÷,ÊxAGNbllTXS 1146+189?îæÖՕb?¦<ûgQÅt?hèË͞?a×SÓý? 	¹˜m?¥þya~ð"?ïš]®ï¥f?ˆ'`.à?D9U˜ñnh?S'"> ?ˆ$þꇏw?‡BN7š…w?¶'ÒÒ?Š'潐]?p.ÜùÊ
.?`îýFS…!?¢P¨þI'7?ˆºå?ïSöô½Ó?wG´ÂÙ?w?7¥E?b,*O°Î?ib§C¸Æ?t‹.r14FGL J1149.0+5924?ډY?·P@Kû`¿]xÀ:¼¬'\fÀ<—ˆü"cõ@S*¡iFÁ?ýØPXÝç§?ÑC¢A2û*?ÍwV	L?ö<py@œúåcǿᲈˆ˜À¿éu0™$ÿ"¿Ô£"ŸXö¿à—¢H"Ä¿ã…WWÕ©ë¿ðAGNrdgNGC 3894?ï4u©yð?­½¢.•¦;?eÀµ%ßY¹?_»Y¢‹|i?–¹47ôÖË?­¬OÉm·B?î속À§?œ¢®þº?bYZÑqË?g
 uðÙ,? rvކ?›yÏA*?íwŠvFXµ?— BMÝ?N?ˆ¥QL`Ò?{þÛÞé|?±/*#®>?"ñ>nW5?í¡f[}?'|4¿e_}?'s
jmA?p…²F²'?°¨Ë!ït0?îÖ×5¯4FGL J1149.1+2819¿ïµûx(R@S
†½ôµÀ;5º>TÏeÀ<¹šTbX@îÎxžwO?ú:73rô?ە̅0b?ЮrĘ Ë?ã ýy¼…@œVUi?첁Çë¼|¿í–ðÝMM'¿Ü¶¡gP¿Òòœ"%¿ä°Ëæ¿ïýYÝl[AGNbcu3FGL J1149.1+28157C 1146+2841?îΦÝÖYš?¬—lùïo?Zœ¶Í¦W?_nѤÂâ?¢@±œãù?«º‡
¦_Ž?ïcäŽ:µÕ?••– '?P»…Š…´?f9ÿl°?'wµàô"?"äœ`&ýû?í&pô1ߞ?žÉG›a‹m?~ë¢{;Õ¢?rš¨ýò%i?´Ý¾6½E»?žIÑνӕ?îØþrÉb?‡J<|3Ä?T8…Gx~Ú?PøúeÆà?¡ÎT©3åâ?†Ô´º4FGL J1149.2+6246¿í'"÷©¢Ú@Juü–þµÀ;C`dÄ¥·À<➽ÅÈÍ@î]ìn@åRº·÷S?Ä(2y$?¿¬'Ó|"P/?啬¿ç<?üUŽ¿öЁ¿âVà±09¿á?-!¡:x¿áOÝO³¿ããY '¬m¿áVó+Ü'¿ïÿÿ)@k*AGNbllNVSS J114926+624333?ï±ûÁ.?y™›ýÒº?cáEÏ®?^oMår}?}'F
¡?v&Œ}Ò?î–0ÃúÃ[?¦MY~ëW?ftöEL®?p½múZ<?¥;¬pïu?¥ØÏß¡vþ?íÝƶËú/?'ìÍÛ4Šg?ˆ'I"Æú³?xT"¢æ?¬ÂJŽžc?æ=ÖQ¼¹?ît]÷ÙÍæ?¥ۘŒ?Š5ì/0?z²oŵ?¢3žôèÆ?‰Àã5''4FGL J1149.4+2441?ì	Êó?
˜@R÷l7`¿]À:îY_æÌÀ<
ª}íl@ ÉêWÍ|?ýz¬(©l?ÎՑ—l™?Äk«õ'½?ùƒX´Ï?ú^/5L¾¿ê{`"¾ŽF¿èç6žË2¿àÖ|x÷c¿Ø]]¾¢¸¿äå}ºŠ¿Ò^(_ÀñAGNbll3FGL J1149.5+2443RX J1149.5+2439?î˜?úòÖ?¥4©Ï̅÷?]¯ú›šñ¼?UP"ÙxÑ?¥Ž€{ùK?¤ïþ }J?íy2ŠÕv?³f›«ë;?é	ïK.?~²:óú…?¯øQ/ƃ?®Ö0=iê8?í̓aŽ­?"÷¬P?T?xÁ•èï¡Ó?l	C_Ù@?°˘|r?'fcˆçŸÿ?ç%ûOvÁ?®œÆHK¿Þ?¤r¹ö@P?˜;Os¬‡ï?ÎKŒ§kÑ?®s}3‡4FGL J1149.5-4029?Ê7=ïN×Ô@4Þf˜»MIÀ:(3û°À<;šß÷.@-' %ú»@lŠÅÁ@?¼†êªÙ2?ÀbHIšÓ«@ÑÄ2ÊW¨@
®"ѶkŒ?í€ÿ90£6¿ÅG³Gë|¿åÓ áŒwr¿ç'
~ß0¿â9ã¡$¨V¿ïÿþó…õAGNbcuPMN J1149-4029?L2Þ´«?sVzՅµ$?Yå{|`L?^Å͂ˆp?{0‡±‹U?pàj+ÑÓ?ïu'<Tß?‹Š‹OÕ"¤?_±äðÅF?p¶MúIzr?Ž¯:®Z/Å?ˆC%óÕ~Þ?îÞÊAɅÉ?"–ZQ¨Ÿ?zÈ+tõ g?ptY.Ì?t¬é'þÈ?%ê6½VM?Ë"Ҟ?€ä¼ÞHÖ?‰I'",?pÚÏ"q|? •cJ®q"?|¡è)ðZÀ4FGL J1150.4+2418?ÔnXdèYh@Rþ€sWæqÀ8Ý^žšÀ;ÿ…ÄÐ	@
;ƒcÍ/@Š82vtÑ?¤ð?éØ?­‹ÊNe!@Ñ™Sù|@
H¿ "_ž?éT¯àÄ¿à
RÎÙí¿äF¼x{¿áº(»
,ª¿æ¤Ùžlg1¿ì~õ†÷AGNbll3FGL J1150.3+2417OM 280?ï[›'A
W?‹ì‡Àpó?Z6ËÈ?RÜ2{Ÿ‹Ø?'ë—«-øí?Š#7Nªg?-­mœ?¨npˆCì²?>4½·^‰?''c'Õ?£Ÿõ»N¦?£cD)Ë8?ïI¥É`V?ˆµF]ÔÖü?tÓ0i
?rQãàénS?š¢ÅÇÛ?"紷Љø?íb
Ò¿—?œ"©¤2x/?®]öV?—*'V…å? ;é½v+?…¨º¹…õŒ4FGL J1150.6+4154¿Û'££@Q«øʁ˜òÀ8²¶d«{CÀ;š‹'!­@"³<Î?ùæ)_tڝ?¨î´Âٝ¯?º?©ƒ	@ãá!îgQ@§‰§´¿Â¢£C â¿ÓvÍ;Ý{Ç¿Ö+P%\Zõ¿ÔjzýÍÙ¿Ü-þ`BµÝ¿ä&œˆŒAGNbll3FGL J1150.5+4155RBS 1040?ïÇEQ(£'?sûœ&ù~?Pòd•hŽ?LÏ"?Ú?x ¾FT5?r m*<ÏV?ï=9*Jó?"}¸iý?cÔÞh5Ӛ?u@Â>??•Þ>éšã&?'O`caì¹?î瘦¾5Œ?'Ïۘ•²ð?'q#aïÉd?ƒ×'èb'Õ?™ÔYwAi·?Œ§Gí¥Þ?íËEh¨7?˜Oß´âQ2?wgwT•?h¨Éå®X?°4ƒG¸ø?˜Ó¾{;Âg4FGL J1150.6-4823¿ì¦•åsÑx@*…ê̒jÀ:,Ù=—ÀÀ<Uäßq@ZT4_®@ÕM¾Ñb?ėܕ—¬Z?铙¥X½@V́Mrz@uOVTux?ïýý'¶œ¿ÅŽ"½"u˜¿è6u¨"ÉY¿ïÿ°NçÄ ¿Öÿïcû}?ïôlj£'AGNbcu3FGL J1150.7-4816PKS 1149-480?ËE‹ÕÄ?Å!½6¡|?æ.R$©Y?ʍü`0êq?¹²eÃ	®?¹G¯dMò½?Ä/'!më?Ê°M–g3?å06ØE,?ѐjYŸLÒ?ÅÓ®#}}f?ÅöðäÛ£v?Ó&€éb©?²b±;¯
·?Ýgõ*Ü?·#"så&?ÎãâCÒäö?­_­ÂIsP?ÁˆcÿÅ\?´œ¢Ùò?ä½·ïywW?Ç4Áié¡?ˁÞ]I?¿¡7¹4FGL J1151.3+0957¿ïcÔ/[|@Pï‡~äâmÀ9î{Üð0À<^RèÛ M@Xx]Öu@9^á6ç?³ê©ó¿ÇuçY?Ùæg¨…ŧ?ûáHÒ©¿å")uš¿â¢âƒw¿ç9iãÉh"¿ß?üoQÇs¿éa[?êx¿âðŸdß©AGNbcu3FGL J1151.5+0957NVSS J115117+095826?írb©µ¤?±úSÝvN?†)yÃÊÃ?}'ÛÎ)ͤ?±ª
ÉÙَ?±I!|Øhx?îy@»±?¦úè_7È?æÕÔ?"üŸK}µè?¤)2[Ïu?¡âÀH½rô?ìW±ÙÁƒ? —²ÐN©?›|Ö2qeH?ŒLüª1Mf?¶hÄ䕚š?™z¸t^Mx?ìñÄV§NJ?Ÿ@JVT?©æ¦ýÁ?—ex´Åk–?¦ý‰'§?ŽïƵúÙ<4FGL J1151.5-1347?Õ;bFœª@GIÿ¼ä!À:+oðSÀ<L•¿ðEx@Fs´N?þ¿4"…ƒb?·ŒÍ|²?°s¿jc¡?ø õäKj@´~wTJZ¿åVÛó[¿Ÿ'gB¦»
¿á×&ø'Mu¿Û{–yS¨õ¿Üë±~è"R¿àþp·'©AGNbll3FGL J1151.4-1346PMN J1151-1347?ﮒc¨lÚ?qםiu$H?Q§­ZØ?Iweƒã¥?')R 9ˆä?p}RÀ':6?ïxãæ4?‡ï¬+˜ïƒ?JSëÖ1¡}?W§'®AM?‹£	£XÐ?†}옻?îðX÷£V?€°0ÁWۆ?m¨…lZ?Uˆsê?>?ž\ßÐ^¤?~ZØ;¹bF?îí`öå*°?zäìS3Ãp?v±2UJE?]æpõ?œ§"úׇ?x±`äqlÀ4FGL J1151.5+5859?͘ä3¾@L>-b8Ú<À9¢àJXçÀ<U¡E@Ý\u éZ?ûY
Ð>?³ ôpTÒ?·9@þÍÐÙ@ÅÈFUNç@OKí"C?ä
¢»Jî¿ßBÌ-jœV¿ÕpàÝûÉ:¿Ý8 z´Q+¿ÙùÄ6%¿ã¸ãÁ…ñÇAGNbll3FGL J1151.4+5858TXS 1148+592?î»­&æ"?•$'0ñ†	?|'J]ÌH?rU@ÓÖ%Ê? ÀDRˆm?"HB¶s™I?ï)Ä úu?•} K¨~ë?jo&§â?tUY{K©õ?—y‹y{Üs?'¬ä%Å?ím²ÔCj?šK¶0N³?‰:—Š§÷ˆ?6q<SYÞ?±knåÀ?•Ü¾(d"à?ì^doyY"?™ŒÂ+í4?'s:Yæ$»?z"'!i?¸p
í»ª-?—á¯õ­74FGL J1151.6-2115¿Ý:Qàrq@CÀ¹w…r›À:üõÊò×ùÀ<–þï^È@ ~Þ¿¤ó?üáX"Ì?ÌëÔWÜ?»k/ùÂÏ?ñµ¡7Ì¿?ÿ8¤aHÅ¿ïênió9?ïò`ŠÚ9¿àh"¾é_U¿Ñ²ñCú€º¿ä
d½™Óü¿ØhÒý='íAGNbcuNVSS J115140-211345?ïš,²¶	k?Ž¦eçRý?Cu±î̇i?@ÐnC/É[?ˆ=x3Üt?à:q&E?ï[–Š~ο?ŽhŒ"ëX?W%iÌQ÷?bd#."øc?"Ød£?‹Ée.‰Œ?î8ÁI÷mY?ŒëËS>Ò?ta*³?_¥GÈ?©çÆ
†£?‹4mÖsà?íg<ø?šw®nŒ?ŠT·yú?tRS·ïB?±{•Ÿ°H*?Žxâ¾îŠc4FGL J1152.1+2837¿Ô%/%͸@S40@9«óÀ;aga8)<À<ć0
‰Ç@!?Žµâ¥?ýÀ(Ê#¥!?ʑ8wß`?W]άÖ?ÁåŠ2ôI@ù
¿cí¿íIn¾¤•÷?됫´NPÆ¿áѲ_c<æ¿áqùAŸÝ€¿¸½=ã^¿ß$ù9{øAGNbllGB6 J1152+2837?ïxKÅÐ?$1œ¤'æ?RºÓä	?[-·fŒmœ?§'œlæ?Œ®âC@t?ï¥PÖ?†êXÍLB'??maÔ?N~2ë¹,|?…ÅÃá¿8?†2Þ1O7?îõ|D?'&:]½Á?t6G»Ö¹
?dxfP£'?­p7°Ä´ª?.zô×?îÉÀ…›?‰ÕPS?hΔ$Òy8?cZ‡XŽ?¢:zµY"?‰Ñ¹N‹­4FGL J1152.3-0839¿ë'Ò`h(;@I¸ÿ!³®ïÀ91÷ÃœcÀ<¨Ü,¼@ïapˆSK@è#½tj?¯
^\N,?µIȔ.@|Úa
@å،s–?»kÂíC¿å;*®)s—¿åÁ »¿å󾩛¿ê"œý|B¿és$ºÊlAGNfsrq3FGL J1152.3-0841PKS B1149-084?ï`yÚ?˜´"ý_[?_Æ8g1äŽ?UþsþŸ?'ÿÊÊj¦'?ÇWCÙp?t×õ³?'wšLyY?Kž:Ò
?YiØü~ƛ?bBH>æ?'Ðè^a?îòqu\Á§?‡CŽ+¬k?uýö­
&?i—ː&ö?œo'Ö¼ˆ©?…Mê: B?ïÊcÅJ?d`ãˆtƒ"?^	…!Þ?KºÙÎ5«‡?sL3ØãÎ?`'˜•ÜÆ¥4FGL J1152.8+3308¿ÈeÇQ…@RÿÀ6âëÀ:œÞÀXÀ<}׺f˜»@§õýȘ@´Å¿'Q§?¾]b wóñ¿½TÂá!Ô¢?þÍðÁ@Ÿ¶2+¡D¿Ô¦"Sß{%¿ìwÅü-ã¿ëÕ9¸ˆr*¿Ò¥ñ7"+¿é(ýOL?³E'Q}¡AGNfsrqB2 1150+33A?ïÀš")ï¤?|9Åtjv?qÿàá;	?sufiF{?keªšNó?pç·p'õ?ïx(܅–Z?'e5+KŽA?WF"áB'?kêAxê?öbjA?#:»fR?î…h{Ï#?'N¦	†ÔH?q-V–?k‡¯Eo?¥ƒÓHPJZ?ÇF—x?ï¼ùá?t±EÕEžZ?nŒS §M?l©µ'Aþ?r=pUo<m?gB#Œ•Š@4FGL J1153.0+8056?ïèfuʖ@Aï îؐÀ:+jК¸À<_ÙSÃÌs@}à}Ù @Zt:dÜ?·hfEÚ*¿¯Œç.¢Õ­?ò×z:XÁb@ꗶ?—›?íº¾?©c¿äÌ°èj¸¿ê8±ø50¿æ¸/â縿ì̼¦äÛ·¿ïÿŸzFAGNfsrqS5 1150+81?ïúA}	"Ì?GÏß`[?@˜Éd0ö¸?CŽ•gÀº?)…	Ýb¨?(ûv.uç¸?ï¹à~OE?rwƒ9;&?@~vÌ­Ã?Tù|‡ƒÚ?€øï!RÄ?€JÀUœÊ?ï"zqÞûè?¢ð³?rQ¬Ú3V‰?f©ÁÆÙÄá?—F"­e?$ïï`á³?ïå_-K9?Uóý¼I?VƒFi›ÎD?H­Æd1l?^¾^ÿò(?OÃP3KÄ4FGL J1153.3-1104¿Ø8‹}³EM@H¤eƒèWmÀ9ð4îõÁÀ<6¶³…Óê@clùþ^?@0>Œ,Ê?·c´Û>˜?²ù¤)ëa?øopJ붝@8ßwŸHÛ¿Ålê¹ò«¿âõ}ðñš¿æt«"­ÿØ¿âvO¿êñxô¿Ù8ÊKéžAGNbcuPKS B1150-108?ï'J»Ql?ˆ[µm—Øh?V
ágèÏà?N¾%›Ãä?ˆëôò®Š×?‡-©(tðÒ?燎»qfl?‡uVßڙw?:Ýa
b5?LzpY·½?…HæV)?†¡|ÄÛbæ?ïM&áì¹?…¼ál÷g´?qMÃþ<%Í?cDȯîÝê?›Bê$3_r?ƒÏ}ë·«,?ïÞ¤åI&>?XéS
q-Ž?@Yì.'Yg?+cäˆÆóº?mDŸ«9+—?XËïŸ`~4FGL J1153.4+4931?à0£«>î@P?W}•WÀ8Þê'ò#À<AÌN!Ì@˜ üö@ŽŠ#Û?¢Ã^äçˬ?£ãñ¬€&+?þäԕîê.@Hm²(‡¿Öыؾ¿äÔú˜¸¿å‹MpÌö¿ãs>í¿í=HËJ썿ß9Ü>YØAGNFSRQ3FGL J1153.4+49324C +49.22?ï‰7ø)[?'«3z²˜g?S×WµË»X?L/åN·ú|?‹7S‹<1'?'e¥Ë$Ç[?ïùÓ?‰Qdý7I?Kÿ0'Q‹ ?dÂ>m)»?†ÊŒri?†ÒLþ¡E$?îÁ)íö-5?"š<–üÇ?vEe½œ¸f?sLÊtKË?¡$´h镖?'M2˜|%°?ïþ'
ãgÜ?0|ÔV™?
":Ç?	>ü¸Ñ´?½œÉgŽƒ?xÛ%·4FGL J1153.6-2553¿Üƒ+…%*@A–ÃÉîËûÀ:…wqP¥4À<mgZ',–@ BP¾ßNZ?ü5 *­R´?Ãõ]$H^¾?ÆÙHƘUL@1æaÉH´@Z9è4¿ïñ¸ðiŠ?ïE®*JVe?®@ê</—Y¿ß)¦W>
¿áÊ°]*}'¿ãž™]´'AGNbcu3FGL J1153.7-2555NVSS J115338-255412?ïÁñ8ä?s|R}ÊÈú?Y­à'žºŒ?S¬?µ?xÌ[;ßJ?qěXàm?ïŒË/¦²?‡ê‹Êû,?PÂM&Ï:6?[œ‰Á¥m­?Š´ê–|lV?…ý¸ç£°n?;/1W?Ž3ÛZ¤?sN±âà?fͽ¬±€Ÿ?£Ë›–ÐŽœ?Œjç-ôP?v¸àç?†«QÈP^?|ÒÑ*ô…¶?huúºä;?¤*.o`Ý?"ý€s>­4FGL J1153.7+3822¿ï©Ô
•@R`{_ïJÀ;i°Œû%¦À<ç¥'lU"@ ¨RÑ^,?þ­é—Þ®w?É´—L?yœèƒŒ'ô?µm‰_(žI@vJ_É¿ï7óâ:rB¿ÊRŒ)nŽS¿Ð¢0aFÁÛ¿è'Ø¥H#…?Ã^jÄoF¿áPå*'¤AGNbllB3 1151+386?ï‹i@Ü5Â?‹r¿'²y.?Gù«bÌ\?EIo	®3G?‹¦ÅÉÚ?Š¹ûӁ?ïU)öºÊ_?˜8ƒ%±Å¯?RE´_¤B³?qUûà²Ú?"6eâ¬oï?–Àýڛ1ù?í°àöÃâ?'›¶îŽ?~É0r	‰d?o!ºŸ+?¨?°ŒlA)HZ?'7b€9Ì»?ï5£ÈìÍ?ˆ@Å;\?M61¥?Mf,ƒËZ?›LaÕVm´?ˆ6Ì_˜®ý4FGL J1154.0-0010¿ìzìÅ»‹‡@M³þCg]ÝÀ:ÄÜ=ƒÀ<:贉ßè@ ¡Øñd?û¨À˜áãµ?¾(²?œ'à?®1´%Ÿ!?óêIš}Å(@ÉÌJØÁ?ï÷±j8X?¥^w.µ ¿ã?@óVµ¿ÔEO_¹£û¿ÉÁJ£g†¿æ-h¹&ý›AGNbll3FGL J1154.2-00101RXS J115404.9-001008?ïZýÞH"Î?Šrž™ñ?Zm6aü?UÓaÑxB÷?'ùsõ\;?ˆå>Š»à?n$6?†/U"S?I»‡Üù?WðïY™?‰Ä+kEôº?"³à¿£ ƒ?îew)bús?")ýßFú?jKÉ݇?a.ú4lÈ?¨Ü=?K?'Þ-ð‡]¦?íÈSrÈ¡?û³À6R?x…v"A?h2BDZ?°5'XÓZ?¶H•ØS¶4FGL J1154.0+4037¿îžµ
y¡h@RؤTÞÀ:KO7u¸À<Kžd¶@ŽeÖÉzÞ@¡·D¥?»©¥Ö=ä½?žçÚø½7?âÙV}»Â@
€#½Ÿ]S?ï¹OýnUH¿¨³oX¨bµ¿áŒÈ›䟿á4Âkðê¿å:c©Ä\¿ÔdfÜØÞ~AGNfsrq3FGL J1153.4+4033B3 1151+408?ïÚ¼MÅ?dPªÃÎg?@K k㼫?3¹l°Á™.?pè½Ë ü*?cÄ0'æ¤?悔êj?…Ç"Îy…?CÔ³®cƒ?SØk4ýP?""q#o?"¤8³¶÷?ï'Aì#3c?|aöpi Ü?hA³X4Ô?T@=sî§ï?˜zE.Œã?yÁTëg?ïE11i0?x×!®±?{ú]Ú¬!Z?cˆSy=àÜ?`bc'ѱ?u•BǪ#4FGL J1154.0+6018¿î[" Íf6@K³û?¦ÞüÀ:Ý]=ȸÀ<FDw(UŠ@ý¤)j‡ˆ@j$aY?¸ÅxqÖ²?ÎÐd¾›‡@AÀ6@ÓÖ;‹qc?ÙêY¥Ã£¿âRƒÅò½ø¿é³ß¿ëÔ9~§¿ïþ{ ۑ?ïêӝ÷LRAGNfsrq3FGL J1154.3+6023RX J1154.0+6022?ïšÅoØʬ?"4߁yÓ?…{¶[T"?Ží•Ÿ
-X?^—oÐ?sf9;y"?íú^aèBv?±²µÌ\œl?Ž(Õµtµ? ½˜ï{ÎÃ?¨Ïät֚?¨ö°†9?ìĆA÷ٍ?¢+\Nï*?§{Ä­2±›?—û´ÄJ³?¬;×3Oµ›?•îJ€"'?ÞtS?œ¤ZqæB?–lJÆqþ?†ÀŒcœu?–=¹ka-Ã?"ùf*¿q4FGL J1154.1-3243?ïeA°»@<Ÿ¡<%J<À9Tm'LžÀ;ñ´#ìn@"XWÚÝ\?þðCå2`?®wE0áŸB?¾ÁÀ	@t\!iT@
¨!"Šé?ð¿ÜÉ/^giq¿áª¿†¾ ¿ÙœF‡£Íпç¨S;wG¿í™šùdAGNbll3FGL J1154.0-3243PKS 1151-324?ïÞãßò1%?'Ùª‡Œ*?Vç	øž?'&
€U#?eºLˆÒÌõ?eG¯'6C?ï.ϔÄl´?–ÿ•Ë ¢?j΢¶LlZ?u§•i8–Œ?–Ì9¨Ü?"ä&Ól½È?î±*•i×?"Ç"•8¥W?js×ìi?‰ì,1{"ø?›ˆ³fÎÑ?†¢õWç¤z?íþ\½Gf?ŽiL¶d×ì?'p´xnsñ?yшÈÇÓ?§aÙïRd²?‰»L-U4FGL J1155.5-3418?â»>ÛïÔ@;%ðÃL‹À:=Áz‰3À<O»S'ÅA@ ³‹WŒƒÜ?ûъŸb0?¿ 8Åxr?³yx€´	K?öœÜ_@Ÿ1czN?ïþ»ýq°G¿ç$O€íl¿Ó¼GÃe¿Ð\¢õ¸Ô¿äbÐzw¿·Bï=åé©AGNbll3FGL J1155.4-3417NVSS J115520-341718?ï¥ÙS:
?yw"<½È?F½Ì­Nå?<ª÷
«°ô?…îîf¨•?~¨üBØ?ï|¿hDM?ˆø†©æ€?R¢‡rz<É?`‰ã‡k?Ž{՝u/?†Ä{Ù}c?îWj66aÚ?'
uó,.V?oâòª?\£!@ˆ0?¨‹3xYJ?'B=q»¹¾?í¾ß‡ì‡c?‹Dz0',?;´Ëo"Å?eªº~èÞ?°Hsä˨?Š?ùHT#4FGL J1155.6-6547¿×8çÛ¤ŠÀR¶ä-;¢À9Ö%Ü2›^À;;u –
@Åv¼ƒ)@ê໗?ΛraÇEN?Õ« ,ZÒ@	WQ:…7?ôxƒ<
d?ïç)€=Ó¿áD7%?U¿é¤óÕORN¿ë¸ðvö£¿ïýwקò?˜cï=ºöŒAGNbcuWISEA J115414.97-654215.0?àìžÃÄ2??Ç4)K´'?·²WôÆáX?·[òª²lŠ?Ø:,{Eã.?ƧÆÂH?½Hb¸Ðò&?¼@lVxö?¸uƒr)©/?ºª£ÿú?éHC: ¬–?À˜>@ ?Í$vÐmõ?«*ðh¬¢?Ââ XÃÈþ?¢úÈÞmÖ!?ãþ:išòC?°LBìBT«?Ÿþ|~™v?€RwSž?Óu¿MËÖ?±E
ס?åqÑ<huI?°÷t\T.Ú4FGL J1155.8+6137¿äbÂ0Là@K!ýÞ½À;˜Mà]£À=™0¾
í@!
øæ0K!?úèÎör¸"?жÙÛÓûÀ?ŵ¡bê"?ö¢XOLnn@)¬'½¨?í#·•-#O¿æÈóĈZ­¿æ×z:XÁb?»òð"wÍ¿ÝÉ/‰Z‡5¿ä,\\×qAGNbll3FGL J1155.9+6136SDSS J115548.40+613553.8?ï/¢
^?'ÃÛM
=?cýúW*y?ZH»¿}?—‹î´}Ï?'3'øÿ*Þ?îìh¡™½?›N2YÆ;k?cÌôrÂt?t?äÖ¨ùc? ª.º<Ó?™(4ýÿf	?í»S>A–?"5knˆ?zY<B`Œ†?j‡ŽÖ"Ï?°ÒJÿêˆ?'óŸQ§ý¡?íº5md@Ö?–Ó¨Ms3–?Û×3±ã?w´¬O‹ƒ?¯å³\ÏyÓ?–+Nñ'.t4FGL J1156.6+0640¿âp;mOŸâ@PpmH÷QÀ;eEñ{ؾÀ<¾Lj;Ýý@HãHº.@q<î×í?Ø
PJ›.Å?Ó5ÂÅ+?õã]gº#}@
Ì3j¾9¿ïõð¢i÷À?ïö$´ë.¸¿Ñ·	ìèÌ¿å
ö~!)¿ïñÖ¤¿î×oZµAGNbcuTXS 1154+069?ïvØ73?•)è'S{«?_ók$#[ç?aKëڊ¨?‹£Ü›mÇÀ?"'<ïöïZ?ïye};Ô?'âö27ïF?V³ïßÞ?l"Q«wb+?ŽÐ@"<¨ù?¸çH.¿Ô?ì>…)NZ¾?ù'!Ó?¤Èw^` ?u탂ƒ?³§›}ùÀ?–cÐwÏ?ïp¶uϏï?{)^h'?hN˜P[ŸJ?_÷j7R¹?¾¼xb?xêÙ¸nØj4FGL J1156.6-2248¿äˆàÜ@C+8`™ËÀ:mAaÊsÀ<_†z%@ð\ñržƒ?ÿ"òXwZ?ÜW¹û8ñ?ÄǏ¡F@"à¹(«@¹
¨4<¿ïÜl²°Â?ïÞÁÉ'¿Þ¢T~1‰:¿á[¹.׿ۢÉä:&¿èG犾4"AGNbll3FGL J1156.7-2250NVSS J115633-225004?ïu|ã˜?öÓJÑh?y-ò—Dó?r/*µdM?•ÅÓú]»á?Ž,({sÿ?ï@¹±3?"O`n7ÙM?caiíM?oüN,+?•|±6"6	?èñC½+¥?íÇú'c~?"Nr™Ùõ?'='{¾¨?t·K¿üzã?®ðòY)?'—@iw´?ì 
ÁA?",å_XZ?—è.iÓV?ƒ(Å%#½?µZÞ]y?'Xñ3öΡ4FGL J1158.5+4824?é蕼P@P—BÃÉîÌÀ:3(¦É-À<…bÎ+qž@iXûÓö@g6:N°g?¸bÓ3ïÕ? ®Ý½NÄM?âÆ8Éu)x@ O¼€ÏH?Ý	ß<fÏ¿äŠLŠN¿åµ‡k™¬¿çµ½A›"¿èWõ¹€¿Ýõy(àÉÚAGNfsrqGB1 1155+486?ïÔêϜ9Ì?ˆ5µ"ˆ˜Ì?G¥¸ <?amŒ '?r•çúω?"sJ}]ù?ï¶yO`µ`?"^+ÓoÁ
?:{vÊô?RPF5=Ý%?C£öñz?ƒ€	õV´?ï¦×p$r?"ó÷M?kÓU©'ç?Uý²üè)?šPº\֎æ?' €‡ì¢?ïï-+"?J•Cþ÷Z?@æÒ, ›¢?0ãJ÷§?YŠ<"¿nr?G¿«"óó
4FGL J1158.9+0818¿ïê=9á@PܵÜÆ?À;ˆCaÀ<§óv"Á›@ 6°Ë9yÉ?ý[ÛÈé~?Ê@åxjIö?¶ºùw]?î<G
ۊÖ?ÿj?›Ü??ï‰þ›üË¿íP_ÿD^¿ÃEyÇAGž¿ÚÚ¨!ò™¿ä‹ÂÁ[)œ¿Õl—£TYAGNbcu3FGL J1158.9+0818RX J1158.8+0819?îåþlOAÂ?˜ìiÑd?Q®ý^¡?GR/:^?¡›Ê;øé?˜¯ÄÏuì?îÈ «? ðä;؍¼?rþšÔWŒ?x=؇?¥£ªåeÊc?ŸÓ&ˆ·8?íÖblB?'™šÇ¡Á?u&%mӐ?b½v8É?¯õˆtÉÍ?èdßHc?ë%¹²\mF?Ä|´;)ò?'Go©û?|?!bG?ÁG0H™(ƒ?EÒ«X"4FGL J1159.0+0939?ӓ|DÛ7…@Q&8ÅCÀ9¼b †ˆEÀ<H}'ÒÕû@B™³šÌ @¥?|í'h?³Î#Žû[?°ý<aNÏ?ü«ÓXI@7}	Àóü¿àD'❪?ÓÚL|°TÇ¿ãU38;°°¿Þs]$žDú¿åÄz¿ç=W^‹¦'AGNbll3FGL J1158.8+0941GB6 J1158+0937?ï×cˆ3pl?tÝ¿¬"I?DÖ¼ÿïf=?Bã"(Àè
?q³dFI܄?sØ^B¦ü¨?ï¢ùzžQ?…¾µ|HF­?JÊx½—R?YÚ N{¾?…"ù¶û+?"B3/'t»?ïG•C2r?x‡ôZmˆz?h•¯¼"e?[Ëa¶œ?"ú¡¢î%?u†y}})|?ï²·hŽœV?gµ!š£?i'¯Yá)l?SXbŽ?yâôÁ@&?b	ö_¨»m4FGL J1159.2-2227¿®Ì,p¤Âg@CjmŒ?À9/v>J¾jÀ;ÃQvëè@–Ÿ¤J¢'@Þ¥rðR?¶fŽ_0½?ÂKD÷Ö»¹@€	ö#l@3M™Þ?׀ÒbãÏô¿ã¶"v¿æ–îÄnYz¿åX³ UöW¿ênjЛ¿ïÿ~€8Ÿ"AGNbcu3FGL J1159.3-2226PKS 1156-221?ï¬óúuÞ?ԉ•÷Ín?hĉ'Ÿ?d=óKÁ?}$i>ȱ?z«÷àµÍ?¤
êˆ?‡b?ÿ¨?N:+øðÂ?_ÉBC)?Šv4=¶Q?…•)u˜"?î¨r\ñ{?ŒÓ'Ì)ʧ?'<÷˧`4?wgjnF²l? éœK—4?†Ü:/V??ï0éª.@Æ?€
ÏÀ"œç?tPIyå?`ìcê_?"ÎÆY刯?~›Ù¡õ"¾4FGL J1159.3-2142¿Ñi©"¸@CÈú?̞ªÀ8ÞqÍ¢µ¢À;¡"ØaV@¸‹Í(<@çüÓû•?ªD?è<.?À·—FBÐ@á¼ýKð™@3®~Øù¿ÛTbWä¿âûîç´°¿å` ‰wãf¿ç9Â,_Ú¿éá1ޟ](¿ïþžÖð<>AGNfsrq3FGL J1159.2-2141PMN J1159-2142?ïŠe_ѯ?†ŸJmŸÙ?o `ͦ†?lg.ç¼?…ž‡ô¡ò¦?'©#ò Ô?îI&)Ä0?£…"ðû	ü?yÆCŒÉö?…ÜtÊØhj?£ÔÔò#³?¡~Y=c?îòÀ	×d?ŽÇÏ-¶@º?'†ä
Ä·^?~®¾·bè?˜dŒÕ'¸?ˆTÐ\ê—ý?íWQ&o?"µSO¿?—U">ÉD?€Èי¯:?®à\î4f?'\ÿ—ù:D4FGL J1159.5+2914¿³ qÙú¶@S˜	¿œb¢À6Ù¾´Ü?À;tR¸3¹@
ÍËzgO@ӎ¢Å'F?‰ÕQðQ{?¯óæÖ¹5@"2~À¨@!æƒ.Äd¿Á8'Ù÷¿ß#½ßÉÿ"¿ã¤Û·K[H¿âóύd¿æT+
oÆ¿ç¶é¡éÜAGNfsrq3FGL J1159.5+2914Ton 599?ïžñb§ÐT?"7'%\?J±,÷ߟè?J¹Ö\
œ£?†˜"†ð—?ƒ°qDøþÔ?ï3ù*©o,? 'Ÿ0H
û?g9""'U?O¡ýÂHX?–™¨_ï¼?ž»#!ñU"?ïF1VÀŠ?Œ¬&­X>?z!œ˜
>?v€õ½Àó½?±–Žë˜?‡-˜5ؖÐ?ïø"	¸‡ƒ?E»A÷½?Ą†_KÍ?é¨à°Ul?I×H	c?DIK¸©XW4FGL J1159.5-0723¿³
m(†ã³@J¢qÿ÷œ"À:&Nɑ®êÀ<M@± ÷@¬úv~6'?üæ/Äé©|?ÆÉGÝc?ÅڿԖÆ@ÖÓßÅp@ò´/œû¤¿ïÿ틉5ž?ïüî×컿Þ7Ó@"TŽ¿ØoE2980¿ÚMâa®z¿íŒ_¿ƒ8.AGNbll3FGL J1159.6-0723PMN J1159-0723?ïÓE§hEÐ?jc'7¾H6?WÖ÷1?P/È`˜*d?pš6Ž²?fY›üÝg?ïlâœ2"»?ÿÚÇ Ù«?X'éé¦?eÃ6áÓ¾?ÚéŽÎ]?.
0"?îœi•£ûk?åtäz?u}0òÇsI?m¸î}ÅÀÆ?£‰À‡gZÞ?Ûk
]n@?îˆ&Tšá?"ꞌÛ,…?ƒëè±ã´#?laвXxž?¢' ‰Ý4Þ?ƒAàS‹4FGL J1200.2+0201¿ÄDkeâó@O–#ûÀ:(*ùÀ<nΠâc7@Ý0õkL@Cx$Õ?½Æ'ÊBXë?½Àdß}©y@jä°a @\wûT¿âõõ»Ÿí¿Ý­† J¿á€>´pµu¿ÛYÄAê¿åSP¦^N¿æd¶}Õî´AGNbcu3FGL J1200.4+020287GB 115739.6+021927?ïÝä§dœx?a^Šƒ0Í?B¬PµÕƒ?7ê³O t:?m›-‡6?_²W†6Á?ïšýÞp_'?‡KRÉ?GÞL3S{?Wû:Ð-?‡Â£ ²èX?†=YGmÎ?ïFŒšcÉ?yHä¨]`ˆ?f™ún|v?['Ý|=ÖS?"[=Þä‹?v¶²UµA?ðBm¯?nÃœ{Öë?cX_Éó,T?IrÍc¯SÞ?‡Á«üçÉY?m+Wj"¾4FGL J1200.6+1229¿êÆn( @QÉD=F²lÀ:^4Òo£ýÀ<v†oj@÷÷ÔãF·@"Í–&?Àíá\Ÿ?¼¥Ú5@)?ùý ª/@
|÷ÔÃ?í•÷ƒY¼4¿äy'"¿å79ó@ÔÜ¿åÒÑɋпå\ÏAS¿ïÿLa¢—AGNbll3FGL J1200.8+1228GB6 J1200+1230?ï¦Ø´J¹Œ?†Õ±x"Y?R/¾–üã=?JoêÐ50?"Ûr¹?†W°Éɛ`?ïn¿Ø¿?Žæ•\½i?S‡ØlXø?`šäK÷ö?ö§‡aHƒ?:"?¡h?ïÂÄaþ?à15µ?kö§Š\?X<>lÍ\?˜Àg''l¾?}6x‹kV?ç×\¾?"±)ôV?ˆ"½ïêc]?rO¼îž?œ—D
6'?€ÂëTr
Ø4FGL J1200.7+2008¿ê¸ò%ÂÝ@Siì,äeÀ:´Ç‰¤À<l´ˆ2i	@Yï`÷'@âÿœ,ñÑ?·ƒÀë?©Ýì@Õæ?ð ó*.§³@	å·Îí?Ên¸ÅXå¿å­U¾xv3¿ç'ù¾ÈR?¿âÛ._ƒô¿ïþ|§ñK1?ïÚ¡–'õAGNbcu3FGL J1200.9+2010TXS 1158+204?ïÍKð@ž?w1²Ñ?^¨™'™S?W{ÐBaŸà?qȳÆ
ë?tPm79ÅÆ?ï[S"Lâõ?• ¸
Ð@?`ìTÅF6›?rù±‹`…Ð?'xݺگ?"c÷zâö?ïºôǪ?"Þðñ+ð?u'Ä"[?kæ÷}fì?™
øãô?dGl¦ì?ïp; NiÊ?}»7¹ÿܜ?ª¶¼—>³?q·Î'º?"¼Žî?r7zS _û4FGL J1200.8-1429¿ã —±{ÒM@GMØ@žUÁÀ:é'm{.À<vRNmS@ VÀ"Ûë?þöíï/Î?Ë«¾à%??¸·²3nlo?ìç¬sßÌ@CIËûìu?Àw¿ïçågÎE?îYœô—ìñ¿äˆ-@U¿¿×vÝâžÆ)¿à¹Ö?è"iAGNbcu3FGL J1200.9-1432NVSS J120055-143040?í'Á6ÍÑ?±ã"S\4?YÎÕ¼°®?PŠÉãV)m?·gJºòž¦?±Â´á}iÉ?ï ­Za¨&?›ÒOwsùB?Wqꏮ ?k€_³Ôì?šs6
ÐÞ?šŠ) qc?íCeR c9?™>óɵë?tï.³ r3?b)s2ÓÉû?´•âÊß?˜Tq¸S­?î0ÝDâ?•þ3k^®7?_²Lós?\çÊóó?­/_Ä#™?•½Yu4FGL J1201.1-0332¿ïwO'þ@L'"¦óõÀ;Ô/—@À<nê™fn@Hÿ¥è?þ­[î=_Ý?̇'™£?ÆÂáfŒÑà?ý¯3^Ò@ Ü2ÆQ¿ïÿÀà/€ ?î.-À,«Z?ìNÛ?JB¿Þ…pí¨åg¿çvFŸ¿à)¥÷ÞÉAGNbcuNVSS J120111-033219?ïr'Y¯?‡úä`©Í?c'£Hž?a!ÈÁ#?Ž™Í}—'?†Mݪm?î͜xQQ»?¡•,ê,µÊ?ri&Zý9?~›:ay? Ù¸ß"´?žŸÿ`ãÿ?íïüC¬Æ?''6é›?€|3'&?o>yå?­Ñ.àòJ?ŽŸËÑʎ?퍇Ù2Ì? fÈó(*Æ?"%ˆo—/T?"lêÀ÷?­ÊJ¡;?™ƒ-Kòè4FGL J1201.7+1429?í°š¿´`o@R7UqKœ·À:'£.mѕÀ<'ÌK@!'Mš¾@oªÛ
}2?Ó?ÅíhN?םÊD\P?ýS'i#°@×Ç7a–¿Öùœ#6»Ô¿Üéwލ¿àѦPaAc¿êC¡É¿ïÿüÚ±'Þ?ïÿá∠ÎAGNbllOM 198?î('DÇi'?±äüiH?sç´Ü$òÌ?zr(°KB?«•Èy?±9f¾Ñ7?îJø++µ"?«wË첿·?ƒPȞ`ò?'Ùù'áé¨?¦|K%¬k'?¦ðʪ_?êO27FYÎ?¦Ó-4RY±?¯AÀo¡
?—O1[I´¨?½åŽ
ü«?¡!æA"#É?îëM™YŽ?Œ®eM«{?ƒÀ…Áûþ§?zéß|ˆ?˜½SkÖÏ
?"R ,ýËr4FGL J1202.4+4442¿ÔI"*>{@Qw#x«‰À;7˜ólÀ<´"!Š"C@§§·§þ@xd"?Á]m
¦‡¿µsd%Ä`?ô
®ñð@/!Û¬º¿ÚícV˜¿ê"›Oe™¿ßŶƒ	_O¿çCO¢Ý¿ã¹Ë¾.ú>¿ïÿÿ)@k*AGNbllB3 1159+450?ï'ûהï/?•B䩝‹?m!¶ü'õì?{š±¥"©?"8œ[£vì?' OßkÉ?ï$/"@?š´xuS?`XºòGMz?k,V®ÎÒ?™nø·ì?˜›€–jª?íèɏÝÌÍ??á¿Ä ?‡]þ¶Á¼?w5œºœŠ?«›çTœ'¶?‹'ôç˜æ?îèÝK3vT?ˆ—Õës?'m	ß3ø?{]I¦=ڂ?™­Ò!›£?ƒOý`ÔpÏ4FGL J1202.5-0528?uÄyA4@K©›ý÷èÀ:+L''ÙÀ<;µ%ç@[§c0ÑÚ@OãÖԎ?Á¸v¾ù$š?Áâôq¯›?öcLŠÅÁ@ztJ»?ïÿýaw¿çßlâj¿ê˜"t¼j¿êzª@/ðÞ¿ïÿv}_Ò#?ïücÈý4tAGNfsrqPKS 1200-051?ïޖ$@¶Ð?ªˆ±|Œ?o	67ñÔa?ªŠ]Ѷ³?3,:ºÑ0?9[ºÊòm}?ïkês O?"Gö¥dþ?[ÊbB e?q‰¯ƒK?ÆsêÔ?o¥FTÙt?î²ÚÞh{v?‹J©b×+?z_öF«$7?sÿµî…?¡†SP¢ä?ˆ™¢5Ly?ïÞ+aÙüò?`c]ÌÑ/%?PHÊDdWÖ?D­Ø¨Èâ?i°9Ðâ:?[êÿWÊïÞ4FGL J1202.5+3852¿ê¢j÷ÖÌç@Rœ;÷'jÀ:h/"BAÄÀ<'{ZqÍ@d[ô@ÈÒDŽ?µg×)È¿¬×ä>Œ
?õD5¹ö0@¡$29c#?ïÿíáoq'¿â£Éh">¿êsҕc©ô¿àyÈþáòÏ¿ã=š)âQ™¿Áù CVíAGNbll3FGL J1203.2+3847NVSS J120257+385147?ï=-ñOs
?'ßëÓØ~2?lÇx9C?m¹ÅH'ƒ?"ÁRÕ_÷…?'§ƒ¦lÅ?ïYøň?'~Ûuiµ?^Lº8d?hž"Ærªx?'Ü«uß>?<Èñhñ?í®gö&3?"4'^E?ƒA€Ð¢ÚR?ràÓqÛÉB?°$—&:s?'gsZ?ó¯?îÒuª¨IÐ?†>§IFWA?wܛóæ??ý̆?•õŠ¼¨Ì?|þn½©4FGL J1202.9+5141¿ÑvBwî¨@Oå¡ÊÀƒÀ;CZPÀ<¢¬k-u"@O€íl@'¶'!%?Á"íå÷K¿´í¤ˆµñ"?õÕÛiGÂ@]Öÿž?ïܲø¿êbÑñÏ»•¿ç¿:¨rzq¿á×¼_AY¿æ¶ÇÝyÃ:¿±?štµßuAGNbcuTXS 1200+519?îÂÛ¹Æ7Ï?½@éoð.?wž'3È?†ä¬ð0†O? Þqv"T?¼aŠðÝ0?îRñø&M?§Íiz¢‰2?zÄü+
ñ?‡:õþF?§…aPX9u?¥(yq=ÈÊ?íЈ–ü'\?'h ¡5¸ö?ƒDúáH—w?r®—?®&7×ä´^?{bð¬7
?íÃÂÅH°E?—%˜[%ûÏ?²¼nlç?ƒzž¸|òw?«{úM=Å*?'ÂŽ´bI4FGL J1203.1+6031?µÈ¿ZRÅ@Kη#îÒÀ9zû¾QßÇÀ<o*þ±K@vò	óï@n—Oß;?¬èÿ¡?³`ËqØàV@^—eóS@	'R á·k?ï7Ÿçòm¿àBD]§ûÝ¿à'Y«m´¿á*i*f¿éV[¡'_¹¿Ð¥ÁۂOAGNbll3FGL J1203.1+6029SBS 1200+608?ïe ʪP­?ˆt'¬­?n\(Cí?f	'"ÑU‡?7¶Taò?…ûÑñºßð?î'AÄsÌ?¥¡Ãj«y?{©eOa?ˆÚA¤–ñ?£jÈÀLS?¢hw(êÁº?ïéUÏLÜ?…Çw«Yõ?v8äþ"˜?r"Aâ]j6?š>ÇÖ¿µ?6ƒÖÔ?íÞà1?"\í¼Gf?¥†Äs6ž?»kB£j?™Y% RÍ?€¨ûï)[Ï4FGL J1203.3+1119?Ú5å%oas@Q¤_ !¸À:ç²7PþÀ<oIÊFá@7½%•ç@9'åøí½?͎8½`É?ÑޚTª|@iåvç¾@Ú¼ñ?ì[²BÝË"¿â¿ˆ¬Œ%¿çŽx¾­¥?¿×ž·æ‹º´¿ïÿù_|è3¿Áœª2AGNbcuTXS 1200+115?îи+ÚP?ºn3o?CþƒN@?€=(YèjÄ?FûCò˜?™g0ð–r?îÎËæȋM?Ÿs'>?t`ƒÈN¡?€¶*jå? ‡1mˆá?›"1šÀŽ?íZõŸv¸?˜Rdß?•¼w)?‡°‹»ù?¯‰0Ýn?'僕l¦"?í™QËN-?˜$¸g?žáM+ðm?‹=÷¤?°*ÕZ'x?"æáòbPb4FGL J1203.4-3925¿çÒS"/@6'‹â÷±}À:?Ï)è1À<INiŸ
@!*øé‹I?üב#'?·IӞ"?p?yùø²ŒbW?Åù çÁÆ@BÝJHy?éj‹#µî?䯂~õÔX¿ÞÀù"æ¯!¿á£œ*Øò¿ÒÜÍ Öy¿Ðå×?—ožAGNbll3FGL J1203.5-3925PMN J1203-3926?ª¨3¯?–­Ýë-=?tѯ¦¹!j?k쫲F?¢ýO`¥ ò?•£°Y=|?ïDxt>º?´¥!6Jz?SÆ>\2ø?`î¯Åò¦o?–4'fÛ÷?Ÿ›†a?í.ˆdŒ^9?˜ž¡ð²ä?…/úaïUÀ?xÍq"Þà?³å½_#…?–,ºç#ü?ìD	§—m?ž=/>¼?´pÍÛpi?~.EݔÀ"?»'Q™֌?éÖ'Énæ4FGL J1204.0+1146?åUÔÖ0£·@QÂûÒsÕ»À:w<
rIÉÀ<a
ž¿s@ ž^/‹2ù?üƒŠ´#ˆ›?ÄE´£ú?ÀRb"‰î?þy*X™J@
¢î$î¿ïÿýaw?ïÿþBe«+¿á1õ°ñ¤ó¿Ö¸_˜1¿Ù×i]ç'Ê¿ê0S'ˆAGNbll3FGL J1204.0+11441RXS J120413.0+114549?益ZÖü–?€ùÓY¤ŸK?Vb[*±§Q?Sfÿcâ$Á?ƒ
Ýäê¥Ä?€MTƒ+h?ïzÁúšé?Žfmuìe«?Y-qä‰l?eÊ&…:@?Ž)Ó7É-¢?‹¤ØñR?íͤʊ:»?"½ê#Jp?yrڒA e?eûu½È?¯÷X0E?'éŒjž?í¨×#]jc?';Ú® 0L?'ö¸ÒŸ?€^Ç|Kˆ?¬w1aQv?wå4FGL J1204.2-0709?ïÝÌ2n†@Jî`RP/À9nsbÎ+À;ÿ;"G@çß†Î?ü«åÌx7?µ#	ðCÊZ?µ—ÈAíá@.º'®›@—`,'?ïú·‹òçê¿äa©0'¿ßÝB»¼Y¿ÑÀ· jÄ¿âå4!Å¢Œ¿Þ•P^½$¹AGNbll3FGL J1204.3-07081RXS J120417.0-070959?ïôC~·fÍ?ZÁÁ9à?&Â5Ü­Þu?$ö(}ˆ?T »Õœ©f?X› =ÂQ?ïq\±ØÒ?Ž"22ιJ?XÑ=Y®?f'Á?VŸ?OÃhA8?‹NÔ¾îDë?ï#:¼8
?ƒ6îrLjn?k£ww™‰û?_Pw£g-8?šg)¹…ÍC?S
 ¾(5?î78,Õ+˜?ªo)8Dš?†¹'æ?qÀ½ÏÌ1d?§zgeÑ?ŠsV¤÷³N4FGL J1204.8+0407?Èú;J@P7!Õ<ÞÀ;?ÐÐgŒÀ<~ÐV©Z@xB÷¡aº@ØÄ$"õ?Ðú? Ò2'?»æ;èך?èýpÇZ@	}=*WíR?惠žp˜ï¿êÉüÙ´¿â~wiÃèø¿ç5Š€Ìï¿ïöþdŠ¿ïÿñQçSaAGNfsrq3FGL J1205.4+0412MG1 J120448+0408?ïÐ" j²?{ß[>"?IfïI÷?FYëŸò.?tÐ؆šgÌ?yoX¼"ßè?ïP³}ê¥?"~¬óH?[»æê…Ï?nä'œ–y?"-ÞôOÃ?'›ûsWX?îkÅ~ QO?'hõ€p\?{N–³©è?rë×°g?¥ÙÕ?…Éã?ŒËXãc×?ï99¸d-?|²¡ò ?oOähQÉ>?_v|BØ?"ô<;éAN?zT¦É«74FGL J1205.7-2635?ÇmW"²@A"÷ µíÀ9mc¨FÇÀ<$
­,*@@SÃ÷f(@¥­Ûp?¯—d53¾?£9F? ô?ñ*MFðP@
cÒÃù"?ãR+Sk¿äå^ÿiؿ跍¹ç¿äNüm¾I¿èñžBuÆ¿â¸Æ báwAGNfsrq3FGL J1205.8-2636PKS 1203-26?ïÇÚSE?ƒW>bä?e-Ûû=t?]¹ÎÐ7R¸?†Â'§l?V	¡z?ï`SL+ù?ˆL"ÁSá?QªÅm~Ð?c#11J?Šr'E'‡?…´ÉÉ÷Ž?ï>ƺ?ƒ6€"©zÄ?p2ô.Ä?c6Áä.P˜?˜Ëj¡?3jWO?ïao?r'hM'U™?wu緘¯?d2"Â2Ì®?€DÐc×ñ?g€Wëðª4FGL J1205.8+3321¿Õ¾7©öš7@S—àÞ҉À:êj€§ZLÀ<'Æp'9S@réîñÐ@
þ`Ï6?Åhî
¿†ý±Wa¡í?À"‰õŒ´"@òý
':¿Ö® ¤»5Ì¿é9ˆ·Ê¿å½Ëb>Ž†¿ãe"bøô¿î	܍40‰¿ï½ A"ôAGNbcu3FGL J1205.9+3315SDSS J120542.82+332146.9?ï,)³¨÷?–ƒýŸ_»'?pK¨ÝÙ?h¯plR?–]0Ħ©©?•3Dâ¾QU?úêÊÈ?‹ÙÓÏ?INÖýW#í?Y`¹u
?‰»ÓÕwÛÊ?‰³_:ßëÇ?îÓVVù&¥?†í!âiv?qÞá_çÖ?ctðsrõ? Ž¾d‰˜¨?…C÷e!^¥?ï'ø<¦b?sÁD¯%<ã?p'‹Í®oÝ?`ÎÏ9?‡.*ï$[?pùÿ'ç,Q4FGL J1207.2-0524?í¨sÃ@Kàw¯dÀ;ÜÂä¿À<œ¤ÁëÈ;@ ™o¬5R?ù-Æèk?֒ÐÝR«ô?Ý
³ö«˜@x÷…@±ü/æÍ¿ìNá¿Î¼?ï{ìàh‹¿Ñöã•Ò¿Ó>úç'Jñ¿ß='üft¿ðAGNbcu1RXS J120722.5-052442?ïÔ}5qá?iVZÝ p?`ú{½»Þ?[ˆ´*"œ?kÓØ?a©™ßÔÀ?ï<Œ‰·?–âÎÔÓQË?cUV·T?p\ÎÂM¼?–Ã>–þc?"¥ÅÎY€}?í¦M]Ø	?•˜,˜â¢¡?l,`¿
?_FG]dƒ?®@R¼?'9£åjg?íʯ§ji‰?'GYSÒ
?‡
ÃÐý?{ÒôõØ70?­'T•Wh?«4\åO4FGL J1207.7-0106¿ÚÐnˆÚë°@Mï÷øʂÀ:"ºˆýj$À<e*F$§@Î]Àz"@ÇúBPÝh?Àø==ù
?ÆÚ9ÝFl¡@ŒXž&Ç@éÉl|«?ïïZ@hOö¿ÑiدY¿ç&Zݜ'é¿á"?B
;˜¿é>ê¡tˆ¿ðAGNfsrqAT20G J120741-010630?ïÐ"Dä?ugRyÀ?b›¨²W±?bßd?‹‹?mTÓ6cj\?l^ÒT
Œ?ï¦öèÌ«n?'ý>´ÜàS?F-ÈÛew]?]"‡H›?"ßi?Ìò?¬ÑhÐÂ?îŽÿ#ËT/?cÁbïUq?ˆ4ýd¤Ð?€ÖG?«?¡Îj!ˆþ?…E1»."6?ïÉ~§ïÖ?c"ûõû–?[‰"Æ~Š?Ià|²ñ?D?t^[:hÇ?`n>Àþ
4FGL J1207.7-2229?åH&IaÉ@C£vfœíÀ:[§ºÄŒŒÀ<e¬9¯@DÛ½€?ÿ¾›ÌyÀ¶?Á7°év?±ô¬¶¬Ð?ñãUŠv(@Š`Á‹Ñ?ïÇ~¿M³<¿âg1g™¿ãåóö¿Ûp°½"Û¿ÞÆwž5@¿æèþ[»AGNbll3FGL J1207.6-2232NVSS J120736-223036?ï³…4Ÿ?u"7Èk¼Œ?P\–¦Š?CˆÄ
?4Þù­?tJ½{7j^?ï£ò\çÂ?'ÐâÕøö?DºÇJ[Öª?S(K'Í!Ê?…·¼Qi½B?usˆ¾?îþÒ@»Ô?… Ї[?f ©Î;ÃÁ?R¹8ªž0²?Q¢Äa
?ƒŽßsàY?îèFÆ5;f?|ÿ¡$¾2?sÕ¼ q?[¶¢¡'&Ë?ž¸Vvæ?|)£ÀH4FGL J1208.1+3017¿î9ᇆ@Sÿf¥P‡À;x+¾Ê«ŠÀ<Пe‹u@!KQŽ½ók?øœ bv?Ô\™`?ПäâBTä?ùÕ¢y<,@\<ŽÑ"ˆ¿ëÀnºÈ¾J¿ïûmÊö?ÒÊM8ßð¿Òk.óŠ§¿áì^Á¿Ô1»¬éØAGNbllGB6 J1208+3015?îÌ"þt0?žAÉ2Ž9¦?d½…ô©Á¦?j5¹ë‡9g?¡ñ÷¿þ ó?¶åU?îÉÙ¡5`Ö?©Ík¨qv?h{_ZëgÉ?ß±˜mw?¡Ú¯öû<?¨œÎAI¬?íÑôR
h?œÉù¸X"?€Ÿð©û¡s?r"Â$)×À?´ýrH0 '?šRTƒ‹#`?ìÆþÀ'Œ?›ELh5˜?j52q/Å?b՗×5šk?¸þÎ`gê'?š¿všsMG4FGL J1208.2-7810?âÃ8DÑ&ŠÀ/d"À:¬#Ï!kÀ<hýwƒ–@ =÷¼d ?ÿjj6Õ#?ʳiäËG?³Ÿ€ŽZÌ)?éõv¤¢X?óŠy?­¿å2 -"¿çâ/jPÖ²¿Û¯~ˆF5¿Ûo/BÄ#¿á@¤Ö
¾/¿å!	ۂrAGNbcu3FGL J1208.2-7810cPKS 1205-778?îðʪáÑ?•éj'·?RoØîî¾Æ?ZxÂç´Zù? _֊x|ø?"¿ÀIb¥é?în G$nO?ªêê«"'?lñ4ÆzSí?uìÚaQÌ?§NèAQuí?ª73†>rÛ?í¡†XW1?–)ÆGbð6?ymG'í?níGÿ´]?±g3fhÍ^?•õ=4Å?é
c šÄ
?¥‰ãáH³?'JlvñW? ã""?Ɂ#îÒq¦?¥X£94FGL J1208.4+6121?ï÷whä'@K'BZîc À;Gy;UAÀ<ãÚ\ØH@þèL/-•@ü÷¢cl·?Á±Ýˆ0æ}¿£ýÛb'Ő?á¨áJÞ @	·ïEÀ¿íÜ3rSοÚ\uâ/_"¿æoÚ•[œ¿â,ûv-ƒÇ¿¨`Ž­K ¿ë

"ZAGNbllRGB J1208+613?ïîØ(8˜­?\ÂoaÁMY?0¬AF´¿f?+=`4¢?^$Ÿ=!uÒ?Z¤n,•7?ſt_v s?ŒïsÐ>?7êeç"?RŪp¾	š?"Tó?Jã?‹b>	ÊV?îãoàê?‰Rs
'§Ö?f)žn'!µ?b'¶P6ÐÆ? et"ßG?ˆbž,×Û?ïÑg½ø'S?e×»¡á??M‰Žc9†?7¾ltj¢?uWHk#?e×tèÝnV4FGL J1208.8-1751?ïNŠv³]@EêÖ¡aä÷À:ë‡ß\òIÀ<~ϙ/çN@x¤ÉM'X?úøihyf?ئးø?ߚOa'C@I	¼AdN@JdJ,sü?ëÈì}—/‡¿ìWàðñ¿ÑƒÞÐZv¿ÜgŸKŠB¿î]UE¬²¿ïÿ韖]ÐAGNbcuNVSS J120856-175647?í'
ôÒ?¨!¶®{œ?Ÿ5rä÷ ??—êúi<?§TvQI"Ð?¡'øŒvØ?ëød~ ?´^ÂÎuQd?¡]Ö»¾?¢Œ=á1>õ?·ôk1>-?®rnî­ÚY?éi,Ô9?¨ÂƎá?±iåjTÁz?˜Ù9þ;É?Á¦[C"»?¢¿÷œÞ–£?窊É=ðÒ?«û—¤÷Ê?¥ÄsC® å?š"
í´³ž?Ëä¸
"€?©æÏEtz°4FGL J1208.8-2754¿êšÿoXÊ¿@AԀuÀ:œ(MüãÀ<añvÐ@ö@ˆÂ‡y†?ü~†ƒ<`?ÔS—VÉ:q?Ó#ç{NÕÑ@Ù櫛#Ý@é?'³"W¿ïÿŸ½ 	?ïî'ð2,£¿ã°E!óé¿Â½§€b¿èÎÁŒ&ê¿ïÿüoQÇsAGNbcuNVSS J120900-275350?ïFæ³všÂ?'¡	ۘ?U?uW(dðÁz?rrÕ.}³?'Í_wðwt?v÷Ñ.?ï3ûIåäÒ?•Ùwō™?jÌ4S'Õ°?zT(Ío+y?–'8Ó"?'Æ…¹eYÙ?ë :ðCV?£ÓÉUºÔ? —êVvŒr?ËçRU?º²3T"Ÿ?žy€Ã7?ìçß#ã½?—DÐîœó?"x[ u?"5òà:É?´¨ÚKO¸?"O"_]
4FGL J1208.9+5441¿è'€4»@N­gý?[`À8¼iuå_kÀ<Bá³
Þæ@Œì‡¨*@é»ðÜw?¡$åhd1?²·z«ð@`"~@'¤¦½ïd¿Õï5­`÷¿äþ'"o¿çñ¢4rοæñùý‡¼¿î™pI>7s¿ïń~ªTþAGNfsrq3FGL J1208.7+5442TXS 1206+549?+kÃI?xÝç*ÈL?iÛI61õ?bÕʈœw"?u,ÜЃB ?s DèdR?ï(—ÓÉsö?¡;OƘ?l…vËelT?Žúî㙐ó?—\V­dÓ¯?™d
å÷œ¥?î YJ˗5?"¸|‡VT?…-…D/ž¯?€bĶžLº? ¯
:¤õ?'Š¼±çš?ïñVé+©?P
Ÿ™7)Î?QZÕo'ÈÞ?Hƒåsî\?Gî°è+ËÓ?<ªEö;ª4FGL J1209.0-4630?ïìS@ÕïG@/~ÀÖõD»À;"G¡A)À<`émƒÐ@0\"*š@mgâghÅ?ÍçΰқC?£ÝT Á?ٟ"ÛCÝû?þ›©¡¤ý?è,ck	cV?ÍYþí[c¿ë7»ûS¿Ðzý©8ž¿â£Ÿ¬Ù¿ïá½?6.AGNbcuSUMSS J120905-462944?î,ƒŒÞ?¨"×[)?j(w8ú!?lÜåN|½?«•?ÍîH?§vyð}?îu†¾A¹
?«D¢ˆj/
?c."»4ù?uåM†5^e?§t±ð1.Õ?ª1<¿I?ìûYEüL®?šC"#Ý&??ŠÍp#œd'?zïlƒ¼Î?´Ë‡Ëª	?—U•"êK?íÈ·æÔÑZ?"æŸhÔX€?…wŠÜó?vïÞ_6'ô?®0c°/33?'"ZôD#4FGL J1209.4+4118?ç'‹	^@RY•ÔèûÀ9¯¡BÛGÀ<N|c'í…@^owG?ý¥óå?ŠZ?´åp‡§~µ?«Û^¸r?öÖ»cý@]–ý]
¿àˆÊ>}¿ãš:Þù;¿à›T\ÈX¿ÐÜÍ`pƒ ¿áf¬ƒ§À¿ê†#À¤ukAGNbll3FGL J1209.4+4119B3 1206+416?︰–ˆÛÌ?qºóZQO?O"¦gÏ+Ô?AÀ¨aF{?µ?î˜4·?p¢rE¸"?ï€1Á#¿¿?y?0ÌÅ?Ry'R@B–?c"'-ZjM?¤]ŒÈÍ?O¬‹l{?î\qVC­?Ž'«QsB?x,ù0û<?i!ÎÛP‡?§3KyèåÍ?‹8x=)æ ?îÙD[ѓ`?'Ð#´
5?ƒ·]A?pVkÜw?šûÅüÊÌ?~S§¬Êã¤4FGL J1209.4+7608?êð¿P•ø-@D\Fà!qÀ:¼¼Š_ióÀ<Ön%wˆÎ@ÿ˜Î˜~ç?üñÊ,ß\?ʃ2yúÂÔ?Ói¢À^Õ@YíÚcŽE@	PålU闿ìëF…¿ºõ¡Aٔ0¿Û·yT¼¿Ü_G£­™¬¿êñ0š¿ïÿJ-J»æAGNbcu3FGL J1209.9+76072MASS J12093020+7609120?ï—*ö×7¨?ƒÎõäa7?rñÔú4Ù?n-ä'ëë?1É_´û¾?}¶×·€¦?ïbԔëè?'-óçªôà?`æE¶*Î9?s"}»?'ˆ¤«½¥û?×Žµ¦?ì'ݦM3?ŸÔ|ᗫ ?¤#™N7[?"yÖóm~?±WF&zã¢?"f´'u¹?ïQgóØظ?x© â'Ÿ?|ÒÒ ?g^b3ô8J?<õz`ã?s™Ø#R4FGL J1209.7+2548?Õ½¯"hé_@T%sBí»ZÀ;|iÃ8èÀ<Õªøg…@1<¼ô½'@9±Y©¿'?ÑŽŸÀz.?»G‹.ò±¹?çÀÞöÅð@Ͼj´SÚ¿ïé‡þ'•ê?ïÏ[½•ø$¿Ç÷D…(0¿Ù·ª%ØØ¿ä?"=ßßy¿ïñ/DÀ#AGNfsrqB2 1207+26?gÔ$?"O2÷áŽÃ?N:ŠaÕ3?PÃ(Ö£=¿?‹Õ«?ùY²?'Êúi!çA?¼U)õ?ŒÖÃÉ?4?JV@%ŸØë?ZSÍäíÉp?‰j¬è[…R?‹"²è¯^?îÑjŽ|?'¥½¦½?zé]y?o<ÙÜü¾Ù?«ò¬?i?'Iá¹³8?ï×î¼¢'?°~ü€*H?}mv/+ã?m6ºN64å?•‰¤œ Âj?}î¿ì²C¨4FGL J1209.8+1810¿é¿T¾•žÛ@S9,{‰
ZÀ9•8¬øÀ<IwëÉè@&ãÏGÑP@'ìB³Ù·?°–1Só?™6&`D–æ?å—4àh@i$ ô+á¿Í{.I"s•¿æD}ˆkõ¿å¹î£·*¿æe̽ÞGt¿èvuþ	ῼß0Q¬pAGNfsrq3FGL J1209.8+1810MG1 J120953+1809?ïƚ|?u[õ	~?AØ·ºíJ?;¢ú²QH¸?zwãa‰Z?t|‡¸ˆ?ï°zÒðð'?ƒá-ä?@ U(!Æ?VÛô¥¥?'×EñB]œ?'îµ"È?ï¯A¼•>?ƒè-ÅàÞÀ?k©-_[dì?YßÔÓf§?šôòëž?'†Ï«¼|
?ïíZy#Ñ]?P½
¢X??Få)¡·…?0dþ>PÿP?]yTmôֈ?LK\QÓè4FGL J1211.0-3800?ÝÔ·Ý|rl@8,aՈÀ:`~XËs0À<b$Óš@ð[Œm·@¶ûú·Á£?Â1²)³W±?Á2Ã6K¨?ÿ"Sd+"Ã@ð™§0†?ä±+¡nz1¿Ò·6B\Eü¿å;ÔÂd"¿ÞC5ߵݝ¿êðj`Æê5¿ïó‡K¹;öAGNbcuPMN J1211-3754?î$âUÊðŸ?²®¾YfÅ?ŽŸ7¬3æ?®/"M2»?¦
âåé?¤Ç~J`ü<?ïtÐÀƯ&?Œ²ÈB4 °?ZˆLšÇû?hgUN,+?zÆ;ý~?‰»ŸI°?§X?2Qš€vµ?jWçM–?woò'U»?¢M_Zäý?‡µþkÿ'?îj »\9?'Ø´äÜf?"VMÀf?q:#£»ët?¡MÍj	r?~âù7~ñ4FGL J1211.6-2735¿ïõ%W8²4@A: _ñØÀ:?d?D¹mÀ<‹h~n›@@ï3@WM>w4?Áï$»v8A?²j(gÓ"ý?ïˆØ¡lKÙ@
©;×òp?¬˜¾A2"¿éµ\8;¿æçKžd¶¿æ—4d‹šÓ¿êoÔ;V¿ïþ§¥Ë×AGNbcuNVSS J121135-273615?ïšàPùœ?'ð³×Ö?bítG­ê?`ÃҎB2?" pd‡^?Žñâ¹v¬?ïf¦
©t»?Ž'¦½ŸÞ?RÉa¹S:%?]''Ê¡€b?'þ¨<5<?ŒŸ´æ¯Ì›?µ5Ò?'EçäRÛ ?t
ÊÀCÿ?i+¾œ÷?¢vO$#?ÕŽá½?î]8¼ÈÎ5?‡ñ)—:y^?z¶JF"Þý?b¼œÞF?¦Õªê  å?†é˜7ܪ4FGL J1211.6+3901¿Äù,B9q¢@Rß`þG™À;Yá'nÀ<ÞÖÜGª@î',èÁJ@ƒœØ{?ŔS»d¿ª?ڜªVf?ä UàÝ%
@-=ÐÆ?ïÎá£0ò¿ëbS².»Õ¿ä+z!"4-¿Ùô¼ .ß¿Õ'äKn"\¿Ýõ3ô#RëAGNbllFIRST J121134.2+390053?î"Þp?[?ªáó/?¯ß?Z¤ ¿ËÔ²?Pe9
uð›?®ñý«¡?ª©À-®Ž?ïŽ|Qm•?†u=S®H?F¯Ë
ßAv?R]«;[ìÍ?Šõïö§?…'u[¹?í˄ˆ˜^?–€¼8`â?päëv —?ZÖ¯)‰R?°•™3©?•²in¥û?ï/iŽÀÝ?'øñv'·?f¼ØÚW?[ŐbÊr?—R¨S¡_?'‰"ÍÈ¥o4FGL J1212.0-2326¿åÔ~.?j@CDQ£"îÀ:_bnŠ!WÀ<N>Ȓ«i@ ²WlÎ_t?ü‰ý_;Ϻ?Ĉ°'Ð~ˆ?»ã8)‹À?ùÎފdrp@	³l`%…?â}E`1n¿Ýy]¹ïz¿âLuĨ;¿ÐàØóK½¿áƒè¢–Bw¿ÛX£Ó¯AGNbcuPMN J1212-2327?ïÒx5æ>?¦*ÕþâXÏ?Pã^
¡šV?€RzBȳˆ?‰®ö12=h?¢*Æ9Í?ï'ðfÞÀ˜?"Vþ§®yÛ?E‹Òó¥Å?Sü_ُF?‰ë)&ÀŸÙ?ƒ*è}?îyîNZ¨1?'7¬gî?l®azR?[ÈAx»¡<?¦–5
EM???€ËÊ5?í—" °€ó?
È&"LV?v¸fÔ¯ÿ~?b40AÈ÷ÿ?±Ûd0øu?Ü!Þø4FGL J1212.0+2242¿°Þ©–'\@T½D¦"À;1	G|À<Ã"̳¢@‹F©\°/?ÿw_²íþ?ÆòT†?Ï?³ˆÝðǺ?ëöŸ™Û@ÓêÎ?"¿ïÿE€Þ$?ïö?ŒÝÉt¿ãI=Š¥
¿ËÉKãÙ-ٿꇥïaL¿×+¢zé«*AGNbllRX J1211.9+2242?ïxYJÜ\2?ˆƒ ÿ7L?`QǵÛRŠ?W>֗$¡?Õ;[rÃ?‡J+/Õ;Q?ï'ýa®*Ÿ?ŽQŠÎÆ©¶?V:à}ˆ¨}?e±¨Nã»n?ŒyK"ÄC?‹¸ÆÚÐR?횵).·?•å|̍}7?‡­¿"çó?}8Õ§Fú?°4žÃídš?"z¤"?îYI¨=`?^Ì{™?–XÃ20£Æ?"L={Ê#Â?ž~Æ#YÅ?ÁâÍó5Ì4FGL J1212.2+2442?ï¸ØPÛÝ@T6éNã'âÀ:ç{³Õ…À<¶tðlå@?EbŠ¹­?þñ
‰U~¸?ÉL'jPUÙ?ËÙ@x–Ó@'åøí½?þkÌ´Îÿ,?ïŽBî's¿é='þ¡±¿ØëxßdÔì¿ì{Ô!Tä^?ÐZ"ŸY¢¿ïþ"ØrAGNbcuNVSS J121219+244130?í/h†oQÒ?¼uÑB"?€gÚ¯o?‡£!—Ô>>?´wÀv—ŽÈ?»DÞÝ_—x?îãÏÎÛ?¹Æm´÷?aôWÉ%ð?–¹ÿ'­R?ªÒs8	í"?¶Âû¸Û?ìDÇùi?¡"lß¿²?™Z9Î×+?'©¾ìö­?·ƒ>¦CŠ+?›Ø¬"Q?íS—^Cuû? a—‹GÚé?…J¾ÅeY¤?"Trá[«é?²¹í57¤ø?³MÁ]°M4FGL J1212.7-1402?ï»|8Æ×&@Gã1üÒNÀ;lk§îÆóÀ<¦®òÇ2Y@ ߪG;Ô?ÿø¶zzða?Í&"©x3î?^ô¼kZàÚ?ý©t"$à_?ïŽ:ºæñ¿Ö¾"š´¡³¿ïÐéÅ?áý'aĖ¿ãˆŸvRl´¿ÞØ⚔kAGNbcu1RXS J121240.3-140141?ﳛKÌΤ?¨®Ÿ"ìvl?uù%{í9{?¨‹¶%Ë‹?p94«u?t¢&¡E?ïÒ£g«Ï?ŠÊج:¡?L]"5J%?_`Ë
É;Q?Å}òÀió?ˆÉ0ën?íµ°ñLJØ?"e@(>è?w§Ê0>A?i4õRò"ø?°×ûҙÅ3?"~™	LÉ¡?înå˜&N•?–µ}`á?ƒ]Wõ"<0?ÚÖBJ?¤:P€R‡°?"XûT5˜Š4FGL J1213.0+5129?цˆÈï{+@P%˜Çâ'AÀ:jQ•ôÉkÀ<°!èˆ6@aþ÷KÑ@pÛ4n?·<? |LW¿–¢÷Äг?Ú¤ÐÚN@ýŽøUç"?ïDž/IŒ¿æq*_Oð¿äÊìB3]¿ÙûÏdÛr¿ã@TN5íù¿Ù"-Qqâ›AGNbll3FGL J1212.6+51351RXS J121301.8+512942?ïTký¹·?…ü¼éØF?j¿mîK"K?_¾¡GáN?'&$ÂV¯?ƒäŒ¥S(?ïx£ÔíR?‹yˆï9C0?Rãà?_
=¶ÞÁý?Ÿ6¸à¯?‰sk›Š?íÿÁŸö1?ïð礄r?R½ÿ8ä¸?lÈ<Œkq?¬Ž@·Ði?Œüˆ*?îàŽªR ?€'¦ÒE?‹õä§Ü"?qÂõ›Ê
?–\a½Û?{0Ím•4FGL J1213.3-2618¿ï&‡]yOD@Aãƒ'gMÀ:gn³<À<U£Ô…þ²@!(GœÌª?ùmóXQЭ?È÷V¹Eë?ÌÁïy%µ@@~$É
%@ÿ¤åÄ¿ïÿî' Ç?ïÿÑa\w¿ÝÇyB=?)*sqäT¿á…¤O\_¿Ù+¡ƒóÀAGNbll3FGL J1213.1-2619RBS 1080?ï€Næ'ä?''ŒètI?cêljÛï?Z$Y·	
+?‹+ßÐ9?€Ž½öF?ïy䗜'¼?v3-?Yo^Û¦³l?iw ògþð?ŽXî=fº¾?‹¹¼I¶¦?íÿכ·?œeüÕºGŽ?Šü
¬›?€í¥_D?³ð¢b2Z?˜'9Nñ…?íȋhGe?•èˆí	ߛ?ŠÇça¸{?x¬Õ«ƒ&F?´`¾ÂÅ?"¨Õº{Ô4FGL J1213.6+1306?ËïØñÚ^—@R[Ÿ@¢‡À9·ð†nDÀ<.z>å@mï@Ec#»Æë?¶oè›4y?Èì$+@Ž;—…Ã?û,;rFïS¿º)ß!Ž5¿à_¾ÿ"°¿ãΈŽ¯Z̿ꮊ!V'Ý¿ç"ñÿ·/Ø¿ïþàEO•jAGNfsrq3FGL J1213.7+13064C +13.46?à÷
°|~?Ç`ZˑwÆ?Å·½Ü©—?¼[ž.°•=?Ӄˆ°²6?Æ	HÞ¦·?ÞªÑjúë?ÐO²ð.?Ù3Ò6(6?Ï·»£µ†?ÀD6B½¹¿?µåŠ'!…?偭ŤÂ?±K_Dù[9?Ãxk?ª8?šØ©?Ɓ7ÊxÑ?§Y§€E)?áô$óÄØ?³ýFDð¾?ÒL4ºŽ¤?¶d×Q!sè?×1÷¤r?¥ó{"~¸g4FGL J1213.7+6423¿ç*PÕ@J9C¬ÅÀ:¿ØCùTÀ<ȍÿ1£ç@3ʗé@K@Y|´†…?¹:üUP"m¿±™Ö?è"i?ö'ÄãÊ?T@
«‡WÎ?áM̧
£¿êŠ~¬-p¿áÌs`ŸÒï¿äÏ:eV›î¿íOÐÂû'³?à$"3ÿAGNbllNVSS J121348+642524?îÕDz§>Ä?°Šk
Fž?{ZÔ×.f?v%"G0?žpTuLá?°>
PŸs?ï#Wd5'?£qì°Kù]?XŽûÁ½×ð?iÔèÑ!)?š#½1߶?¢ó´M'ùá?îfÅøèg¹?"Ž"=9ÚÍ?"XÖ-•?Iáh|:ñ?¤Ž¼[Cù?'`+Ýt³?ï¡ò6â?p©!S>%Ö?nKÄ`—?]c}XS»M?ýPÞJ?jԖ.u94FGL J1213.8-4345?ìlL¯!&@2—àXšËÉÀ:Jr}ËÞÀ<%)Wèb@ÚøžaÕ]@¹cc}?Ä[ãÁn?±Ó)]F'?î0kؖ/?ú¶[
í©f?ïðØïÿ¿éÄÌîZ¼¿á6sŸ_l¿ä‹«šM¿àb‹"¿ïÿýawAGNbllPMN J1213-4343?îÊn@ÁQÎ?˜o/®;?n–¥¨âq?i5ñ–)Û?¡oºiTû?—€àQÂ[Ù?ìs}Ñi¦?µíph`?ŒßƓû?''^O1?¸àõ{ä«j?µO3IÁ?ëÇ9)¬áû?¡¡uyûg?•$ÚC)"q?"ï<b·û?¼}!΋
?žø'­»U¾?æÿX±ß?¤K
÷!äÞ?¨	Ó
!Ü?'ž½4Gx?Î;py
?¤¹.ïÍ
4FGL J1214.6-1926¿àIÆÖqCî@EJ8Ÿƒ¾fÀ;;÷'À=¢ÌHB@ài4!Ö@€\FQóé?ؼ‰ˆª^
?ïÿõ^'@ÌiegÊ?ù…hŒ,¿ïšÇ‰W'?ã¨	3…hŠ¿Ö‹¥»ç¿îD´š¦ßÓ¿èB½—¥¤¿ïÃㄟ6'AGNbcu3FGL J1215.9-1926PKS B1211-190?â
§ô$"?Ë
‡lÞ@a?Ï¢K՜P¥?ÇXw™¾?È3Yï?À"Ç;àËM?ΝÀb埌?˾,5£?ãï#ƌ)?Ñ*8ô"!˜?Ã"ƒ/Ð?¼™gßLéì?ãô±ÀU?°5™ÈF{Ç?ÉÀî6àt?­œ$ªkÁ–?ÆlJÉÓÉM?£ÑBh0Zf?ž¡‰?±¶•è`?çæªýt72?¶îS?D÷Å?µNoñ]?§m푍®4FGL J1215.0+1656¿æM˜Åfڈ@S2œ#·•-À9x™sÙìpÀ<C?»òn@ÿ¿¼îÞE@!	!ç±U?®ôA¡?Ÿ|æ
C?êêú~Ù@'³{"†¿Ð/Ú¹š¿ã ^l¢¿å-¿öût€¿æ,£ÌùBw¿é•}
Ú7¿Ôe™¢Rû¥AGNfsrq3FGL J1215.1+1658TXS 1212+171?ï©á¬D‰?€ïèؕ¥?LU[·"
–?C»™–ý}Ç?ƒúqÙv@?€â"è©Tû?ïµÄ¨w;?"µ±9ƒ°±?6ì
eeô?K7üÅÐ=g?×™"ç×?"
à±Ö*¯?ïLœ›æQ?"¶•'19Ü?m½»ö±•?\"ÔmOZI?š>´í­Æ?'à"êt¹.?ïõEP4jN?CH/ÄgÎ?1¯øÍFð?#ß{ìÿuf?Q	Ÿøë?A'TOPç4FGL J1215.1+5002?åLéâ 4î@PƒcÜHjÓÀ:†…ÀŸÀ<sŠƒ| ã@ !¬zúÝ?ütA…ÜMs?¹ß>>?³kAþŽL?úâ$íö@@	f†ã¿ë…e?IìÞ¿×f'|E˼¿à.jáö)½¿Ù~˜¡ÌîׅܿÜz>à¿è~ú1‰æAGNbll3FGL J1215.0+5002IVS B1212+503?ï‹(•ÞWÏ?€Í5·S¢>?aŒ¤§"k?UðWŠÃ?ˆÒ±^…1€?~ZΠΘ?ïV/ˆ÷\]?'o­‹Æ}?aB'Wѯô?lv•Îâ?"¼¶>t?´®~Û?í궟ÙI?™z
'y´?€´a<Øв?kÁ‰qÙ?­'}³87>?Ž
Û4ä5Ã?íŸM)ù7ù?'ŸIT-[0?'iZ«°?'_ðݘ÷?­Vª³¨e?^w<Í'54FGL J1215.1+0731?Û±·UŸÍC@Q%¼¾aÏÿÀ:œ¥ÛÇ;"À<k
€òç@!OŽ%óÃ?û/ã7r]?¾9 PB
?˜0':±š?Ý-o|@5ÜiM¿ï¥˜Æï¾?ïã€}"Ô‰¿ÝXcg™¿Æð»ix¸¿äw,ò§Q鿾yĒÁ³AGNbll1ES 1212+078?ïÞülœ'Û?bá?OÏn/?CTëFÔ0?;´ Çbâ,?l.sh«o{?`¶j|5³†?ï¢çl'Çi?ˆááAQõ¨?JÙ>gsA?[Ðñ‹Ï?…˜øÕN¬?‡í­˜?î&¬¹S?ŒÄÿ¶b6Ê?u+üUu=?`SROŸÜ?ªï´ã¬&¨?‹*Þþ
øì?îjPÓ«g"?‡Çx%õ˜?"œ÷72W?qÕÓr0` ?¤3´÷}À?…ÁšÇÃd4FGL J1215.1+3513?ވCœs#õ@S³Q¬šþÀ:׶6ˆRIÀ<–µI"ˆÁ@Îbÿÿ'@<ewS?Æ¢
S?ºÝzÐj?ð#	"ãÿï@lÿGµ¡?ïýl!'J@¿äž‹`Æ¿B¿èúàŽµ:¿ä îzÔ]¿ïø½KO‰«?éÓÈ3àØAGNbll7C 1212+3524?ïo°ozž	?Œguå™yŸ?q'!úÒ?m'êb2£?‹†Ð[¿?ŠÍÑcŸp?î=»sŒ?¨6ò>½³?€£>Èí*w?‹ªÛbÊÖ³?§û€‹ó™?¦°ŸOÝ?ír°¯'"Ÿ?"ñäRï±£?Ü¦!É»?"£™@ßÑ?°®å¿:3?'¸¥~i?î
,EZé?"ôW×}ñ-?ž%Y™¾¢k?‹ä~ªm? ŽÝ€€/?‡mí£y(ò4FGL J1215.8-3732?ïµD@æû@8ˎ\NµpÀ:ØxFÜÀ<h)à¤&@o›Cgß@Ö¢óµo?ȕè41_ô?²
M`Ûâê?ë%ˆ M?þùr奶³?ïÝÐË_ƒ¿åä¶Î]Ç¿é®`Ðû0¿Ýgzbœ­J¿ÓK' Q¿ïþÜIA'rAGNbcuPMN J1216-3734?ï˜*w\?'óÞ¢o?`sÓËL–º?XÒN˺°?›ÐòG¹?'r°eÖ[?îÑ͝Šü?˜n"\-|¹?gÙüÄÀ1J?r SóÜI½?¡e†aÛM ?–JLT—Þ>?íj¤ƒdˆ1?—0t²?O‡Ú°cØ?pUޅ4í´?²€ê酱ö?"ý¥{;`æ?íV>YÆ¡?–<»
ðà½?ƒ)Ÿv'–?w,3WG¨?²èÙBøԄ?"ùZß>mä4FGL J1215.8-1733¿ÚKDc©•@F=Â;yRÒÀ:F¼—Ëc@À<H…7È@N´©‹Ó@ú0bžZÉ?ÂÛy¸Ó›ž?³Ffdÿ´?uøª¡@—EôÖ×?ïiæþÒ-Š¿ãã
ìQÍR¿æDڐå×ê7@Þí¿ïÿèþ†®/¿íÈÔàl'ÏAGNbcuPKS 1213-17?î¥Þž%J'?¥Ko	[?"-µ`)?€i"gÿ®?  Ê°hÌ?¤WSe‰¨?î?–ä6¢ ?£d±iÃz?{œÖiHñ!?"²¬`Uf?¨'öïl·×? ³ûõ?ìí[	¢>?˜¸ÄÉìÞá?•GÆñ&?…A¸÷@h?³Cguö¤q?"è—#C¿?ì²:±"
?•âÀ•ëb?¥úسN©H?Ž:B«8?®á|;y?‹Ž(­úc4FGL J1216.1-0242¿îõÚx9«%@M{›€#¦ÎÀ; ÆÞvB|À<›'–FþÂ@ Ëÿ)@k*?þobð ?É'dÈ×tÆ?´¾¾l6à?îcâÞ1#9@Y‡¼ÍPU¿ïÿZ=¹?ïêâ—9m	¿¦IøŸ¿ä|â((¾¿ÄŒùM3e¿â=)¡dPAGNbll1RXS J121603.6-024302?ï›Úø¾I?'ØbõÎ?KÜY
¸Œ?E÷÷w?‡K|?á!?^,%Q:™?ïps×^B†?ŽŽN…—?OfÓúé'!?^Íq­ìfø?öNt`bÀ?Œ¦¯Ù|ÓI?íßî7p&ª?'ÝÁ]ߌD?yäJÅUâ?kíDlqû?®Ä"Häê£?'ã'CD×?î9ӇÄ}Ä?' -
P†?qn¡äM?j3"Kîµ<?ª4óG5Z/?'šº	4FGL J1216.1+0930?ìh-èèٕ@Q Õ{Ç÷{À:bSåZbÀ<|ërl.@ndD"D@#~Ýx?¼aU"9]?ªþ8C'$¢?ð×*à¼?ÿ†k5X'¿ïð'Úb·…?ïS(Ü¿Þ¨»àì>'¿ã™Á§Õœ¿äƒ×ûÔø¿¾éÀÎfÕÍAGNbllTXS 1213+097?﨑q´P6?yfvaė?]þGÕXl¢?UóU½ð9?'ژ@äª?v¥ï
W?ïYCN-À?".'%'#E?`iMü
~=?mû›"'æÀ?'Ês–¸˜(?'bfŽÓu%?íÌ4t¨¬y?'p{¿"5m?ˆ_!‡É?|YžV'ë?­$ØíF?Š½J¢ì?î.TÞýÌ?'7.ûr`r?›3Ðo-¯?ˆ•L‡š"*?Ÿg3±Þ?ƒ"™Œ[Ä4FGL J1216.2-6121¿îÖèæ͘¾?ó˜2ü¬ŽiÀ9Ü»‰®jÀ;(};•"@•þYŒ¹@͒Z
7'?Ðùn
Áà?Û¯žS<½ö@	¿v¢ôŒ.@ ÂèóI?åmíät‰?¿á}S³{j¿áÓçþ×`ú¿îO
`;¿âzm"gÙ-¿ïà‰B37AGNbcuPMN J1217-6113	?Æíz¡ ¢é?¾ïý>½Ñv?°Dø¸Á.Ë?©Ä2&Á?è<@±m?Á9nŒó4é?¼²šç3n?½6)ÝGS¯?¥!¬=°åÆ?¬J$rÖ?ë'ß>Žt?¿Ü7 $~?Ì6®mˆ°?§¨"ÃlT@?ÂFÃ~ÏàÂ?£%%  ñp?ä`£…¥£?¬â¾ÕÄ n?¼¾þ»íÍï?Ÿ¥Û¼ÿ'?¬u&yts?™òó›8)?ê ÇV®ý?¤ — ;—¹4FGL J1217.9+3007?îǍÑB@Tƒ×Ûô‡ýÀ7ÔÄèÒ½À:ÝgD²·x@ýpÌÚ?ýªˆ>•g?'H]+?§¡—s¡k@6ï^Èt@Δ$9Æ?îg¬sßÌ¿Ùù{Óë¿Ýç‹z‰‰¿Þs¨£ø˜-¿áJ'Á¿Þç=[«!AGNBLL3FGL J1217.8+3007B2 1215+30?ï~}¹-N?™Öˆn˜Ÿ©?Cѵþ®qv?XYæ»JÐ?#£1ÉŌ?˜öȗ¥­?ï/+Ig^Ç? Rõ—Ӑ?hÃlXàœ"?|çQ:˜?—)Gø‹?zÎûxÖ?퉊%ô/?¢;;cá%?…C¥3I¸Â?ƒ¬»[%2?±¿g'w? ÉÏÀ É?ï­zXÂ×?wY}Jˆ#I?Pêᅾïå?I)åз+?'ž…9l3?v°ÅwQÒ4FGL J1218.0-0028¿ëß4¡ÐÓ@NŸa»úìÀ9ûKиê˜À<0=áÄ@b÷Æöt@26 M}a?»®ÌÒ|å?¸`ýµ'?ùhöHÇ/@	i
؅½š¿éã_•'Í?ÁríÒ¹K¿å^ïäÿÉy¿çՍ@öv¿Ú">þî]¿é¹¡KêAGNbll3FGL J1218.0-0029PKS 1215-002?ïqn¢l?ø¥Ûê¶?aú©cW÷?†…€Þ?‹%ˁgV?"Ññ3·p?ïxÀ«=Ô?‹I[ "ü?N¡Rhàp?ZöðPuh ?åÀ
0;?‰¨Õ™‰s6?îÈv0Gª{?Š¢Òà³6†?yQgâð?qkµ‡q½? NpÉ+?†.iø'/ë?îœ
­Ÿ•·?‡
Q\É?hî	ú_õ?n‰é&=?¡ä飈'?†Ø؜*4FGL J1218.5-0119¿ïkšÍm¨ò@N;gäçïÀ8ÞÚVùÀ;©É™;¥È@p¿#¤@-;¢m}²?¨n'>´Ï?¹3©û'†P@À2˜À¥@ÌÒÖüü?ìïÀÛå¿ÜÈ¥ߙX¿áéÄ[å¿áb©B"	¿äës`¿çôþÅwAGNbll3FGL J1218.4-0121PKS 1216-010?ïÓ©:køÅ?m÷ԆG#ä?EiìÏãļ?@lX¦–M?s~%0%T?lÇWª,¹?ïz1Þ©\?ˆ‰\¢µî¯?T—DÆ÷|?a%7! ­ð?ŽàŸÕ€Š&?†ÞŠ`ÃM½?ïÇøtƲ?‡ÓàÈ÷?|ȇk©U?xÑqÇ)¢?–´ß|Ô}?µµ"ºng?îátm'ç?…'èt
"Ë?s2C/l?a0)ό%Ð?ŸëJ70?"ÞwŠc.ß4FGL J1219.0+4827?á	‰œ@Pñ<64À;d‰èK®TÀ<¾©Ü¡V@àÕ:Y˜"@](¯Fª?ȤvçvF¿Š­ükå›?‰ö­›Ú@išÎM?ï`¤&ó¿æBnd!¿ê¯s?è£B¿Å
GÅwÄ¿ãît½A>¿ïÿf¢¡U%AGNfsrqON 428?ï‡,ÎQá?¥Í›=' ¹?qœÈ"ŸE?¤øõúþmÊ?…f˜‹¡¸Y?Šø!Zïn?ïå§2½?‰j?&_›G?F;ßæÄ(¤?Z:¶È^'b?Š¢Ø5æ?ˆ'ÊÓ+_?îõXN,?'AÑZ¤_l?{`f,Õ(¯?h@{…$R?«sÃäàx%?*šT¢À?ïn®x†Úà?zßá¨Zs	?n¾]ûµeQ?``ÁZ®[?Œ¤Ê_[îÎ?wà5†~De4FGL J1219.0+3653?Ûò‹ø
,@S…/D')‰À;oP–À<Îâ*,#t@nx‹¬ñæ@©A­Iz?ÓÀQ>a¹?ÖÇö8Öá#@÷P™u‡l@B8!°º¿çt]î$?îo^‡ŸÇ¿Ù£½l²†¿ã2HQ¨i@¿ïûñH¿ïë6ÊñUAGNbcuNVSS J121915+365718?î%"Ï?§Éà߃×?'M1c©\?ŠVuùþz>?¥%uêÄú?¥Î¥@Æü?í!i^aœ?µ÷˜@Ë??ŸXfl…ûi?ª™ÓuC;?®=6è¦è–?«\æS?ŒÛ?èç—ô`—Ð?¨'Ì[?·T׉Èj`?œRˆ¾ãfo?À·4i™k? ›à¯ÌJ?ê?TÃm'?¬è¤¹n´?½zèœ.H?¬úYëæQ?°tÞû÷A¢?"8ƒœ®Q4FGL J1219.0-4827¿àBÁ ô¬»@,#ÿï9_À:+3ªQwÂÀ<>J—ÓƼ@bxqÏ{@¹m	Ö¶?¼jgÒÍõ?ÊULù	ð@âÑ¡GãÄ@ï¾'˜uW¿ì	ì³!Ÿ?Èx¤&æI¿áå¢áìď¿àÆY`nº¿êÁ¿åԐ{æ˜AGNbll3FGL J1218.8-4827PMN J1219-4826?âÚM[×Ío?Á`vÀ!¢#?˘îaG:?½Â²nŠ"ß?ÈýÜ/†ƒ?¹ké
i'?ë¢(²/¤?¹^¸ÖÂ?¤'5ëUm?¨«µ?¸¦xú4Ê?³R
P†‰?è5°ÆÆXÜ?°¦[£"C?½f*ê*æ?§TIq—¡/?Àv'oі?¢:	ô>ªQ?骒]<ªæ?›Æ¼Ì€KÜ?°"' PÊ?ÿ"#õŒ?ÁmK=,?•‹6÷¬_4FGL J1219.6+0550?æcÓKcx@PÙ¼¾aÏÿÀ:êÒëʾÖÀ<–"
>@XÜüŸÜ?ÿ'ø½ì_9?˼#.XX?•_¼~?óF«ë«µ%@E9ÜœH?ïÁCâWùf¿ä.y$¯ò¿ßõ]¨)¿à{Áâÿ2¿äL-4ìp׿áÿÅGAGNrdgNGC 4261?ïô&;û?"9k¡y´?_ÒÙèÊ??U>lo©?aSܸD?"£b¬ä¥¹?ïKÀ|Þü?Ê5'nÂ?U2Ý]íÅq?]ó¤"uñ?•4ÑڅD\?&–¨jã?îÄYì?'8#'Õ7?s܅}ÍÖ?`µ3™)Å+?¬¸.
Æg†?©z¾½Æ?î–Ñkäo?ŽÕ; mW?"®–<îW?qˆy t3×?ª…§C²}"?.5äQYÏ4FGL J1219.7-0313?»«Ó\LËÏ@MYµÜyÀ9õÍXãÆäÀ<7"U²¹ü@ Æ2ÿ±§?þL(²¦°Ù?¸DÛ&VÖÑ?§(ÍÂ?ñ
ÿˆ
ûÝ@+«	X™I¿¾¶x¢~¶¿ç
>¢¨!¿Ü'|ÉV¿Ü^-ØÖ¿á(aNcæ¿×	ýDcÝAGNbll3FGL J1219.7-03141RXS J121946.0-031419?ï¢ÿ›C=?$þ#ýD?QDSÒ
ø?C_´ûèÅ?…Oõ¸4ï«?}Ö
ùÛu4?ï''X«?v­9
Þ?LH›M¤'ë?^ÃcNkXµ?ºö&Œý?;äÌ.b?îõñ™Ò"?'åËWWa?jJìbk!?[f·`E²?žD@xK?€_š|A¶­?îN-¿½½?†æÐñÇÎ?z½ÏÆF®®?`Ü(Ï=»Ú?§Åt{;NT?†0`'¼eÞ4FGL J1219.7+0444?ï¨,°sa@P˜0O‹YÀ:Ÿ܉Ù2À<rœ…dž@ 0]E«Zâ?þÚÝð,M?Ä˒ûoÍm?½håq´MO?÷ÚÀZ΂¯@—ÎxèI¿ïI$i¢?ïü¿ÙŸC'¿Ð3VćÙÔ¿ß«Ø ër¿ã¨bõ˜ñ¿Îîï¡ãê÷AGNbllNVSS J121945+044621?$l
?³ìX,·ë?€µpu8
Ü?³þýO'i?rÂYã¢?hyN…Í?ïooÞþÉ]?:ŸalÕ®?YQõgFls?hkØ\
.Š?|äɲmŒ?¢Cåþ?î2Æð:æù?Ž¿¥Þk04?w;«àE('?eÿÂìxV?©ì€HëV?‹£¯×Uƒ¸?î;SÐ8?‹=ßÑ@?ÜõŒesO?{jÏ_7áº?£ÜLHàBí?†X1+ug4FGL J1219.9+6056¿ãJÂG¸¦@KãEŒÒ
úÀ:ìdoa'À<͒…©!Í@&ðڞ@VŽà3·?»{ÚÉðO¿´á%Ž?øeLöRØ@ãƒJLÕF?í4VCÙ¿è7…½Äœ'¿ëË!{û¤¿Á›!Äuæ6¿ß؜cÎ[˜¿ïÿõEq#AGNbcu3FGL J1220.3+605587GB 121716.0+611442?ïÙL'f¥µ?qø€¡Úݔ?Tc–0ä'[?MÑa6÷I?l¢€è	å?p;¡‹•¬;?ïØMu|?Šd"£ÛÅ?I>HÍmEœ?Ui+´ðl?ŠöÊ&E?ˆûSQp?îݹÝۑ?‹_
¥h¬:?l"ªbQ¨?^ bi´®'? c%|!½?Š*ß':s¢?ïi^
?{®ÚÒ?wT¬·:?ln~àE?‰Ùý~Kv?uf¼!š_Ý4FGL J1220.1+7105?äÉ#tú(@Fèdìé¢ÆÀ8¨Ê^]ƒiÀ;ñY¡\º@R'Ž7»@'a|ÚQ?£9hs³?ÀÃøzût@­'w>$ÿ@ Ú¨Ø{Ø¿Ìe{Yè~¯¿ß?YÐ,¿ãÒú
w·È¿ælfû·›ã¿éÍ•I¨À¿ê7@Iq8AGNfsrq3FGL J1220.2+7105S5 1217+71?îÀ£GÉôè?´ˆà™}Öê?…'Eo[N? ÷AÁ…±¼?*ty‰µ¡?©ô}6Ûgƒ?ï2ËT²¾¶?¢Â){£Aë?WæQâ'Ñ£?jF¥ö§û?˜(0K~ü"?¢–çÃ
ú?îÀ/^Rù??–¸R±?†7,‹Ñl?"¿—PQá€?œÞ}ï¸f?"æ¹èUÉH?ïêÜà{Z?Sœ\•98?DÄè"›?8¡js·?_ãÊüÉž?P'(›ií4FGL J1220.1+3432?ï=™Ï'"·@T»ìª¸¦À9áéÃ}˜²À<pȖg"@°˜a¶(q@l÷¢cl·?´زP\?®¼œVÉw?ù³·‡Á*@	·nN<N?ï"ÊÀ9¿Ü…SÜ¡@¿âÓŠS«¿á¤…†"¿å>þ]hã¿á,1·20ÕAGNbll3FGL J1220.2+3434GB2 1217+348?ï×ÕÃEIo?~ Á¨%¥?Dì5éàrH?Iø'{û$?qw— 9Ñ?{·áå\o"?ïƒ)Ìd?ŒYpyæ]_?Sˆ÷¤c™í?b§Ì!Üúz?ŒÄ›ÆÀs³?Š/´ùëî?ï6áz¤+x?|‰¬¶¼Y?i¦ø'ðîX?`‰÷-!Ô^?•îñ¦|s?yФ à?ïnµaô?û_çF?ŽVer©ê?xfæÏÌ?¦öš¸ª??vI¦"ê4FGL J1220.2-3713?æüA±"Ç@9;·Ç'
1À:?ÐW›ÈHÀ<`«l)ôÆ@ ã(å?þT·Æ«K?ÀÖ3hb??¼,žïnã8?ý©ÙgåÂg?ûkcˆ»zë?ïûG¿1X¾¿àœÊr/ȿޔÒ?R{M¿Þ@)È¿ÜjÈéÕF¿è]'ømåAGNbcu3FGL J1220.1-37152MASS J12201982-3714137?îé†?"?"»NXՊ?q,¾íö^l?f‰bUÒ½?ž'|þ?'vS²ç?íM¦QN¼?«ãÕñ¬´?"\íw»ýº?™ž¦Kâi?°»'›ë?¤Äþ÷Ì6¶?íGV·«{!?™»T'o×?"㇍5û?s|6«z?³(ÙPýgŽ?—<î7äy?èKEBj?¡ët·ƒ?¯úh
Œ§?"}K¶Çÿ{?ÆÕ9ã‡Ìz?Ÿ3¥~ñ
4FGL J1221.3+3010¿ß'äëôÓ@T¯ke©¨À7ڊèü®<À;/jWWÖ@ Ó]<F,?ú£%"R? B³·[? ³~µßî@ƒy³J@a· D%¿âSÇÝúœ"¿Æ‹sü|ô¿ÜÁ¿àáW¿Ñ†±_ˆý¿Ý—|ˆçš®¿Ã[Â"¹=AGNbll3FGL J1221.3+3010PG 1218+304?ï¹ËX¿?'7EÃaò_?>Àòø?aö£Â¡?€—"8{-R?Ž/š,O ?ïWÍ/Z™¢?•VÛ"¹â)?a—†ÝúÈ?z6'}z
?'ÓiQQd?'Š|åÉ?ìÄ¥/VúÚ?¤D'/Ì?z§€?|rS?xWíÂ4OS?¸0^Pb?£²C‹ µZ?íê×ì¬Ü? IÎ{¦'û?…óZ.Ñîn?x@™d¨ñ ?´Z=úÀ[Y?žˆÏ¶˜øº4FGL J1221.5+2814?éС@Š'H@TÒ//˜tÀ8%\±À;¶i©çÅw@ò®¸dµâ@A(¿<?—`°Þžu:?•š'Ç!?ú/<-­¸@çuXǗY¿Ý—m$E¯¿à¼J~Sm¿ãGüMÃØ2¿àvÚ݆®Z¿æþ\'ÑN¿â°–5a
ÝAGNbll3FGL J1221.4+2814W Comae?ïÞbVqÈü?j
‡˜%‡?.f.Ñ»?)<ZÝKK?o·IUÆ»?iY	?VŽ>?ïh~úU¯?˜Þ½k.?TYŽBp‰?d0懋{º?'ª—1# ?˜	w»ô}?ïHA1\Î?ŠJûgíú3?mל…­{?hq"xåÓ?š<†C°…?‰g]S{—?ïô·v·Œî?GeSËû?;ÔÕ1,£*?6¤Nx˜?O7º‰5ö~?A>:!î­!4FGL J1222.0-4121¿Â¹¤"ŒË@5+ç:6\³À;R[LVñÀ<žË'±ñ@Û®Š—s$?þ鬆Ü'´?ع¶…Ä´?Ó¾-b8Ú<?ùÕt;;?@äïp¶Ç¿íjΪó^?îž8£NN¿â/0¤ãy·¿Ùzˆ|Ê=¿ìNOÿFǐ¿ïÃn_E°AGNbcuPKS 1219-411?íÖ5YEQï?¦ð¡Å¢ô?DÈãxí?ˆLäžT½?ªz©9$Ÿ?¥9Ӟ=
*?ïAä§Ëq?"*_fä)?boG—€?q¡)2Ÿ?•€b±%?ùRå­òØ?ë¨ÞQñÑ?¢¬×F?¥²õvÍ?Þ.XۍÍ?¸33üÝ
ï?œ'[qªÜ?íî˜/Ä?•n?ѝÃ?ð£:Až?rñœÎNçc?¬šU^sX?%IoìH4FGL J1222.5+0414¿áL²P¨A±@P…à`þG™À8©åÂg=À;ÁR4€:M@`5C-Ò @{íx:¤?ª	*\[0ä?¸ªê¤ÏÛ@¥åNë @R'{ÅÉ"¿Ù€	e.'õ¿å‰>7s3Ô¿ê$úö«Ãh¿ë©%þ—J¿î]¦Ùóü¼¿ïô[¼¿8AGNfsrq3FGL J1222.4+04144C +04.42?ïë/ñH±ä?_G´Yr—â?D^ªmûí?@C×)DZ?_qe9?[øŠË3Ð?ïO>]² ?šþx¨8'Ž?fš†]ä ?‡8‹5½c?"[¤ã}ïŽ?",2(ú@?îºo³¶
ì?'Ó7úT?­ÂˆŠ»€?z0o¹mŽ{?ŸÛ(DùD¸?Ži`ç[T[?ï²
Ç"¡?pµ_~Ò,X?q¿cÑûñŸ?f›©žuáÏ?u9¸¤:='?bØÔ¡$1¥4FGL J1223.0+1100¿ì8W«žºý@R#ƒQX¸(À:èâ©­ãÓÀ<'Üo×ÿ0@çQÛiô?ü¢\¶º<?ϲ'´¤ã?̯ÀâÞ±ý?þæ"/•ð@8Ca©"7¿íœºëù¸¾?¯Þcß3½Ù¿çÖåŠ2ôI¿ÂÀbX¯o¿â¡¬ÃB	¿í"M!ÆÏ2AGNbcuSDSS J122307.24+110038.2?ïSz-Í/>?Šï*Í®[¢?^$œ$Xž®?T)'í¢°?"®p"Ž†?‰ïŠ*ê¢B?ïvwómá?2zÔU	?RÊpM¶"?^T'1w?Zl)ï?ÂÕѺ?íåwÃh#?'¡þdsÊ?'Fau_ˆŽ?q9Cím¤?­ö¶q›°?"€â†
Õ?íÓÅz?'ý#¾×¥C?"Cœ?u$þXvH?±þ–|4?'m
4FGL J1223.3+1213?Òçs刎@Rm®ˆ*ÜÀ:Ü<I\jdÀ<d É8Ö@ãw¾RŒ@é§;BÌ-?Í]f"â?¸†›:…?à±¢z¾¸@ámÛhò¿È–œd$AÔ¿å"«=0¿êî±##·¿ÕO*u¿ï¦Òœðf/?íI'w"AGNbll3FGL J1223.2+1215MG1 J122332+1208?î"^ŒfO?¦tL»ìX?'sße?‡PøÉ_]v?©YúV&aÚ?¤z Y"?ï+9¦Ý›?j• a Ú?b)§‡9?n8—c¡?˜ZӖ3ea?œ?	Çù$?ínüÉJ=?–ž§ßSh?ˆSÕw®0?v¶sC`{?±…O:ÿ!¤?"3¯(?ï'¡àH?†½}-A¦?u`²×wM?h:¦a3ÚÂ?•³É×A j?ƒÃ(ž²·4FGL J1223.5+0818?í
ÍÈd!,@Qƒ±mÀ:Å@ªÀ3À<Šéåˆ@ ׬NÓ?ý–:iˆYÖ?ÃЎã³F?·¨˜:	?õÕêî ¬@	nÀ
òwV¿ïû5•äs?ïÿ¢bô¿Ù·?œÎ€¿Û@G¿é=A^Å\?"ÄÃhõãAGNbll3FGL J1223.3+0818SDSS J122327.49+082030.4?ïðä?PÛ?Tp´'¦ø5?7Z~¥5Ò8?1ýc4µm?XaIØÔ?R†Yìµ£f?侮õ&}?…î'ÖD?F_£OÈ«?X—Qœ1@=?"mȁní?"x†ƒ)?îþkØeœÐ?ƒÙÚx»E?o;εOæ8?itzâ$D?œK¢iN?ˆî"<ö?ït\,Ϛ?w5CDdÃ?nŠÅ_øþ?^º;e¿Ñ?‹EvtK?tU^îå4FGL J1223.6-3032?êä¸oóƒ@?ò'B³÷À:Ìsí7¦_À<~ã¬bå@!âv"° š?ù"»¶úÓp?РS\žfˆ?¶çxŸ£ô¼?áqºøŽòw?üHÈK2ÙF?ïýœ"Šï]¿á¹ddIV¿í½÷|£¿?á[æ°£¡Z¿à-ä>ÙZ¿Ñ"î¬ñe3AGNbll3FGL J1223.3-3028NVSS J122337-303246?îT¾ý¥ë?¤ª·%¢?MP#™]2?EšZ¨‹a§?ªJSÀ,Æ?¤‰˜j:"¼?ïSò¨•@0?"ƒ¨jHu?ZZ±Ô¸è/?lž¼t¦Ç?"ÛÿÐkx?'ñJU(7l?í®ØƒU†?œõû¦@?yb†"ݱ6?s|ŽvIâÄ?µ"`Ù·x¶?›`6?çá?ìÀØ]Ú9B?£.-Û`öú?ˆgw"›¦?‰=&ù2f?¶ìN «z?¢!IÙòj'4FGL J1223.8+4649¿¾'åÚhœ@Qda¦
EcÀ;ŠRuÚÀ<í±jp·"@QP=/5x@Ç¢ PØ`?É|üÕÔ¿Õ>bŠ?³ÝÝ@bp¸@°"õ¦o?ÝCiv¼¿ç'Õ1\½¿ã§gž¿â1_œÈù¿âdµ—&¿ïýAt>–>AGNbllRX J1223.8+4651?ï,ÑLî?›9†Ò²¿(?d›ò±@?o/¢¦õ¼?—ÒXvè?™šy¤‡º?ïcÌÅÉp¼?_ULqÒ?If‰³?V°¤ã‹?'»7*՟æ?Ì"TŒ?íåCÓËx?"–\Ânø?{•Züé-È?h¸‹
Šh0?®<@c&"Ì?"OYæTª}?ï-ßÙZr?é3îqIÖ?læ`×_S!?\áA¤?–§8¹ÅÓ³?…ʬιê4FGL J1223.8+8039?̅ø…•ß.@B2u¸eÀ9dFøâÕÀ<®=•ŒÅ@^.$*¬§@ð[|þX`?¯¤b ^.ß?ÀE™'7Ð@11eәp@
<Èý	€‡¿Ýe[#'+f¿Ý)Ucߣi¿ã£C_1¿âøû^°¿è9îlȿ캫ݓïaAGNbll3FGL J1222.7+8041S5 1221+80?îßô)x¶˜?–]Ér°ÐÄ?ƒÐZ@*Ô?}¸ôXpå8?šq'£É•?'8åçp•ô?î9åæ7Z?§¸|{Åòá?†Xo†>Â?^ÿƒT?¦Ë…Ùhƙ?£ñÉø¶}ì?íÙËc'…"? ¯`sx$­?œ²žÍš,Á?•Pó1$E¬?¤	úa
]?"Ú¬Iˆ?íF¼Ô€}?'3]œò;? ÄÚesN?ƒir‡42?ªÙùͱ"ã?‰nh":4FGL J1223.9+7954?Õ˳HRW@B''͖ À;Q,50"À<ãQN§-@!Ç&Š-jò?úâ_:øúR?Ζ[K«$?Â58†">?ñÇ7a–@Qõx'â?ïÊýê¦ý¿ëÒ§7E¿Ó"MA§?J¿Ø݂'™¿¹T÷S3-Õ¿éh¿§J\EAGNbll3FGL J1222.7+7952NVSS J122358+795329?îÕ³±œ
¶?"âcàaö?[i³'C?Qß,ƒ'q?¡ÉwI¶úe?"zRóó7ù?ïã÷g÷?–Þ:¤ì í?\]«.Á÷ô?p›vAóbÌ?œ³Ž&áœ?•€\ÜúšÜ?í†ËEöéÐ?—o²! ß?oÞ©n.C?ZœKñðQ?²Ê°"×?v?–Êr"»¸?íâ*÷ŦL?˜)NRZ‰â?m³d%NÕV?cåYŒH+?°
 ¨Vó?˜…AO24FGL J1223.9+5000¿à€«6­™´@P¡]N°À9¯£¯À<:ʄóð'@³ªºG@YÀª›?³3Áù_'?ÌÁ³éüÞb@-nÎõ@þû¡v‡Ç¿Ì^ÕùFRu¿à4øÀEªÚ¿ç܃ÄE>οèçüÓû•7¿ìÙ@¿ïÿß´0ÕAGNfsrq3FGL J1224.5+4957SBS 1221+503?î™è&[ìÆ?Ÿ
Ðz¸[?¡‹Z¯Î?—­®Öí&?…kÈ3š‡?Š¾žk<?ï@ÓâÜvÉ?•ÓAHž¡F?dñ.+Â?p¥üÝ<·-?•Ga^«®§?"¥ÕØÇ´6?ì²d {Â?¦â¤£‹?¦÷fSÒ+?™$b•ƒ¯è?­â·G¤qÀ? ;½Yd?ï3TkD`q?€|=!ů?†
óê+¿˜?r}œˆÆ^?ñD¼$h?vÔáJ'ë4FGL J1224.1+2239¿äiÛȚõ@T—W'ŽžÀ;^ÆùN5À<¨§<‹Â@"p~]?ÿßCÇÕí?½Ð­¬ö¿"ãL@€?ýáçÌ,"Ý?ý%.»TTk?ë˜> N¿¿íA+®Ús~¿árߪJ¿æž©/"¿ÂúŒ¤¿ÙƒöduË^AGNbllTXS 1221+229?í¹<D'åç?´A~H#É?s½ #)^"?oÆò'Ó•?°úKÙ6:ì?³ÕQ>"|Š?ìxâÅoÀ?¿¦ñÞ«? z5õ³i­?²+"zÿ'÷?³ûÎÝÍ'?¶;g~ǝ?í0ú|
šV?˜S8m9éƒ?}[瘚?p7pa£¦…?´¦¶n,³Ñ?—$Ïýè?à€Lò¦z?¿–ˆlºÙn?£Ó:T ƒ?¥-»©™1ê?܅'#P.ú?ÁWd5ØØr4FGL J1224.4+2436?»­ÐS¹@TÛÀ~à°¯À8ûDæ¹ÝÝÀ;æàyQûu@А'‰Úà?ýג"¬Ó2?¨³×]tzP?©²Ð]Œ3f@ç|¯Ý©@¾wä"?ª¡;¾5ôó?±qÚbâx[¿Þw†®‹¿ÜKêd7b¿ãŸ¥'(^¿ÐjiÀ¸íGAGNbll3FGL J1224.5+2436MS 1221.8+2452?ïíGäÇÀå?[ìð"w&Ú?,âݶª^¨?C[.×Ú»ã?`éí\ÔtÛ?YY¬IU"?ï¨Ìº^@v?†ƒ£ÝáB?CўF'Òí?Y¤¤74##?"·"Åw?…;8Ve#?ïNôHå?…Mµ'Ë_M?n
}89#?eÏûÛU©Â?š´}®/Ü?'î9-Ü ?ïÖLÔB°þ?]_קO?IÂç÷‡?7éÀÌïñY?q¡8ü%b8?[¹¾©}a4FGL J1224.7-8313?ì
•k9×À4e¿œb¡¶À9lʍWkøÀ;ü¢¥±ÕÑ@®¶â)Ö@Ø©_	zÓ?²¦_¿r
"?³¾õsµ'?ývqüœž1@
!+˜	K®?§]	pl#À¿æjW®Î¿çèGçöÿ¿éILÌKž¿åÓ´EíJ¿ïÿË&Ú_]AGNbcu3FGL J1224.6-8312PKS 1221-82?ïè"z›Uì?e–a7Èu?>KCîŸ(Ú?7÷ËXʑ–?c²æÖ.*?cÈý/e?ïˆ6÷°ÏÝ?Ž/ëÆEz?SKñ7Ú?h¢'?‹ˆß5¥%ë?‹Ãˆ'^B7?ïùˆ†×?CÙyGd½?nßår[¿|?cPÎù,ÈÒ?˜"ÒOã­+?~ûpeß3ª?îø3Nùï?'>±w`«Ê?"U/¬=?pžÞš1~,?–Ï`;Ó?|©iüÐR«4FGL J1224.9+2122¿ênÍEn@TjWÑx-8À6Y‹zՉÀ:üÎqèz¨@ã™%ÖS^@9{úLaØ?'<cï¤Ï>?§|€Úš@aS¢>ƒÉ@#؅c¬¢¶¿Ð[¬Cjbõ¿â{R¼ev|¿å¤«{Cm=¿å³@ߙ-¿çÒ(@æпäâÀ‰Èk>AGNFSRQ3FGL J1224.9+21224C +21.35?ïnÜ-*
è?Š¬õmÍ8?R6ÓG$á?QóVäÝjØ?'ÆíŠ0™?‰ÑvXt?ï9¥œï·š?¢û¸0¹?lÃSšÎù?†¡àö¸?•HÓ÷•²Ð? Q¯ùp½S?îâЍŻ.?"™AIÌp(?}¸ÝÈú?|
ø'4ì?œ7èÖ[j?'zý~Kà?ïþv°š?'ÝW[*,>ös·4˜À>ù³Å'u‹ž?%ÑpgÈ&?',¸{*…B4FGL J1224.9+4334?àzµÊ	h@R-gôÛߏÀ9çÁŸr ¯À<•ª¨µ–O@zýÕÙ:ï@kh¢×0?±ãˆP m?–œÇ nM?âF$!Gxe@ÁçAî
¿Ò1žBuÆ¿ä,4 ˜ü¼¿æ§‡-†K¿âÚ|îh(¿ë1Ûz¹×¿ïÿúŒ—ÓAGNbll3FGL J1224.6+4332B3 1222+438?îØ:+\±?ŸµÛñ1}?‡h—Kk™?€Dü݁"?™oH×40?œ!ùIÿå?î‰ú×ZIJ?®{ìi¢îf?†oA"p_²? U@­žàÏ?¡Ä')?Sq?¤"VÉÖ/'?ë¾°3b?¡Õċîæ†?¦@ü‹ÙÄa?"™'
†6—?¶î¼8zò·?šH!C8#Ý?íØҚ¥?…¤D:ë?ªsC
Qg?šÖã×Òºi?ùknn?zš‡œ‹Ì4FGL J1225.0+0330¿âüj´©ÀX@PcJ¡!À:Fþ»\bÀ;º2ƒàʱ@{õ&]6è@-{~%ŸÍ?Å>éõ§Œv?Ö,Ôz¿d@Q)`Kš2@×ͧS¿ÒÏß[š°p¿àìJ«õ¼°¿ßªT|ÙðL¿ê eêV ¿ë68Ág"ã¿ïûµ¸´AGNfsrq4C +03.23?íÓW΢°?´ØàÕaÙ|?€|&<×ýV?yUüÐ 4…?®«y†¨e°?´cÿM«–?ï}/ʋ½?–ñ!"'~Ö?dü"¬"­?‰Õ-?‹}ëˆqë³?Œ^ùéšÿ?åù‡úÛV-?¯<šÏqæÔ?¹a>&%Û?Ÿ¿ºÁ«<?ËiA€Þ?©¦-e^#É?îÞ4ßÝYê?Ž8	ÈyҔ?[ŽÈι?QsÚ¿Ñ??¡D}‹ãðŒ?"ßQ¾4FGL J1225.3-3446¿'Éßίj"@;Èä†&öÀ;;ª]6;üÀ<›ÅPä@ e;Ó÷Ž@òü¬Žhä?¸xƒÚ¿¬-£ <G?ìnƒÖ¹µ™?þ¨XÓÖ¬¿áo0«¼²¿åT[זT¿éjêŸpž#¿Öö†oj¿ÒfuÞÝq¿Ý""ܯAGNbcu3FGL J1225.4-34481RXS J122534.0-344737?î§Çbé#k?¢Ø¥ÊyÜ?heW;B?[¦%(Á&?£ý4]¼Õ)?¢"»s95?îí¿È8L?›ú¦|m?dbØHDÀ?t$Ëør‰?Ÿ»«ïííI?™D£Ù=°v?íá1šH¡ï?'ã`_¹ù?uËÀ~!¬'?aáöŠŸ
?¯3nK±«"?'Ò¸B´¹&?í7˜Áý?›®_3²?vôeŸp8?nÁºèœ8?µí8ßù?›Ð>¬Î"4FGL J1225.4-1550?·ÿïˆëIÛ@GHf^ê–À;Á_0ϬÀ<ÔL~]Óñ@"8u¹•?óv ž9%?æT~!nÑ?á–
˜à66?ÿw¤as¸_@—|Hzî¿î¹6b<¶?íkawê?ΞŠŒ‹i?íêó((Š¿Ä õÙ`ƒù¿æåfâOAGNbcu1RXS J122525.2-155251?îükGgr? ¯ÉFÁ1?€#áÐʕ?ƒÂ³ö>»?˜`¦6g?b!pðe?f"?'
o³£>3?Qgêl6†?sÅgÀ‹-Ö?‹
|)1.?Ê",Šè?ìîã‹[Ê?Ÿgq5ˆX?‰®Æjäc½?{:`µëÿ?µY0H•7?œ"¦Á'¦?ïþ,'Gt?ˆ¬`êÃëo?9…BÚYk?QVõÚl›¢?4JÄÛWÊ?ˆ…«ÿ{Bó4FGL J1225.5-2851?åðæÅFp¨@@Õc¡ À:……žÙÀ<\>ª_º{@¾DVñÿ6@¢ÃÉîËû?ÎRÚ'C?ÕX"Ì@Ž-À,«Z@	OS;;jd?ï¨3PD¼¿ÚYÞb÷F¿âQ žÛøº¿ì˜Á‹¦¿ÙàÀI±¥¿ïüvÄ AGNbcuAT20G J122515-284956?îLl)H©æ? •FÊæ7Þ?~­˜é±™Ø?~;Ô¯Ki¾?§cŠN?._?žoŠX`Ì?ïx[)d?™éÛÇWS?kà
ºœ?{Ž³'ÃÚU?›ÔòåyQ‰?•ÉÒ!=‡?ì'›°9?¢		zúëû?¡w5±
֔?Ž¦yʔŠt?¶Ä'ë?›"*yì%=?îlÔ!0–?‹œ¬çv…?y°¬ýtR?kS
à…¶?¥ü¨MP$ø?Š:ïÈçÞÜ4FGL J1225.6-7313?ëHÅçÀ$é³ÃçÀ:0þæ$À<&A
çI@jђ"Q‰@0;7äs?½ÊÔÏû€i?§:{Ñ݂Ó?ïô&­é³@	JÊ©†ø?ïý•ø$il¿ÅÊEÞÜnÖ¿èÒ»YS¿×ª½®KØF¿äç¼Àæ¿ÜÞùÀJÞKAGNbcu3FGL J1225.7-7314PMN J1225-7313?ï3•œ÷U?'4"V:?JjFA¡ý?G'zðÛ?˜¹ú/…‰?'­X͈Á?íB'a¨ï?¹Y…5Vªµ?HÃAP6?[›Ê†¼_M?µ»^Û2ê?¹:‰ãü?íÎù¿µòU?—k|÷þ?uèlÚûèP?güÉ8w?°)«4 ®Î?•µ»Ü*?îŒ9̪Õ?ƒB¼¬d?z?g_é?c5¼M4c?£ôoˆf±Ç?'•nì! Þ4FGL J1226.0+5622¿Ô²1°Òj@N4oÞµ,À;ªß<;À<ÉLÙÍfP@ÿñº—ëï@k¯–[ ¸?Åta¼2 ¼?iDúIÚ@JæýÐ?îÐó7š¡¿èá
¡~¿åáOp€›œ¿ãâ*⬲ü¿äÁt‹Z¿ïÑqÛÖUAGNbllSDSS J122602.81+562254.6?¯)(?'AÒt?T°=\ì?Q-kòÔ «?…¾ƒLŠc?ŒÙ³§ço?ïwܙ#î?Šp¤å÷æ\?HÛmó>?VýƒöNV?='ncPe?‰Eݲü»?îJö0]Ü?Yؼ8¹?v«Zj?d?4`­y?¨ŽZˆÞÒ^?Ž,S5õš?ï•ÓÝy	?o†M'ý?k#4X	©?V»ý®aXì?ƒôýòœ»Z?l5a±»'Ã4FGL J1226.7+0637¿ïúXã4Üð@Q+OKD¢À:ƎyªæÉÀ<-†K<@!? &¼x?ùUɯáÚ?ÈG•*tÝ?Â[–ÿ‹eú?ý@|&©@Ç`QN|¿ïÿÿ&¦³?ïÿýç!é¿á3ÅP˜¿Ábº_aåM¿ÙVE'¿áYgŸ÷V¹AGNbll3FGL J1226.8+06381RXS J122645.2+063906?ïr÷°Oq'?›Œûíó>Q?Eáyp•¸?R®'‹ø?ñþ*'I/?›-]È<t?ï©]O;P_?" ½j\ÀD?CïŽA?R
~ÇP4?"i³Ö<ï?ƒڂqâ=?î5"nõŒ¤?"»Èü®?m¿©&NË?sÄÖ0m­Ý?ªÊ¾~G0Þ?'Ð-%d®?î'2Û9»?‡Óð.ýü?pƒ™âZÑ?b0#î-?¤Ü_,K¹?†énºY4FGL J1226.8-1329?´²}zÿÄ@Hxª*sÀ9‹}¼ÄÀ<¦†çæ.@LÒ*?þò]€
×?¸[ìÿŒ™?¾#әŎ@PŸ}i[@Š Õ¸"¿×y çÁÆ¿è7k§^¿ÈI?9%æo¿á€`"•¿ä¤&Eüd¿Ð7œ'"mAGNbll3FGL J1226.9-1329PMN J1226-1328?ïÜ¿žÝr?cÐ"ÑÐÚ)?Gf¡ÇB#?A àJ?mf¹RO?b5[…:Ž?ïnô<Üì?"I»ìÙ?Q "v?_¬Wø
—?'vWè?"0Uì_¨?ïZq»Ž?"È# ²Ü?lI–
µc?gÈZ	œeŽ?›«µÌ‡ã?'{T›7GØ?î–Jàlû#?…spS@cò?qáçüKr?[ÅÔy`œÎ?¤_ù¦í&?"‡}']#ä4FGL J1227.1-4437¿ïð–PÂm×@2­}|,¡À;,‰ËÆ=À<šé+¨$w@!8 ¦n?üËyæuë?Ìc¶ˆ½©C?¶dt^Kº¿?흨;ic@ºì*
?Ÿ¿å­4¡Gbë?ï©3g#{¿êŒ5-w?Ö©aãŸÍ¿ãÈÊœ£¿¿r¬šÓ+AGNbllPKS 1224-443?ïÙ̃3Q?l·6
?;5?0/¢L·~?'ȹ‹}?ruŸ™¥‹â?l=øñ'y9?ï¹ç.š?øüO¡p?:«ŒZÑ֙?L7¦Af&	?€°Ý—]ÊÚ?€¥ÊW›¿£?î†Ïº¥Om?ˆ:SQ•?gñ¹!vô?c0lƒ˜?¦èӚ?‹Ô)ÛR?ï^µ}xJ?§¥Þ¡?_ÏRà)6ª?YK5£Å2?',gBNcp?€(ƒ†f<¾4FGL J1228.3+7521?æǧä,‡?@DØ	þ†ƒ<À;XèQ'NÀ<ý
)N­ã@<…—Y"†@è1AÁkp?ÑPÂœÇÌ?®Ùx_jÒ9?×w*#?P?ÿÀwÜÛb½?ïò…ÞѲ¿äʬ+l•U¿ÏõUҚl¿ås`'¿æ÷œ"/¥	¿¾[WáAGNbcuWN B1225.8+7537?îû—ðÂÑ?"E3"þÙ?Z‹'I"ƒ¡?SžyÝÙ`@?žäHÃ
"?"«á…¯T€?îÒÖJV¡¹?œ¡
Õä?b½»bèvÇ?pS2ÍË?¡¦¿¤g\î?š3ú°²]"?ín\¥pÊ?—;DÀŸs?†H

kã?zn-
Ôã—?±Äv‹,4?"»°ÿ…ñ¡?ï³DÊ=¤?ƒÁWL9?xÉ1ó¡È?iÍîäísœ?™—Jéñ"À?S©Æä¨34FGL J1228.7+4858?å;u 	@PíTK±¯:À9òÈlüÀ<PhÍK@áîÇôK@xéö©??»vapD?ÁA;ß,@ª#9Àëî@Þ<)Ñàˆ?ﲋ£6ÑM¿æ|zo1ç¿æÕ*Ÿû ¿ì%yÁâãå¿Ýì%!øxL¿ïÿjÿR[AGNfsrq3FGL J1228.7+4857TXS 1226+492?ïÖ</¬ž?¬4c±-ß?^ZIx?"§'Žªo?j–¯t%??¡âeÁ5
?ï i`×\?"$LG	?Fƒàµîî?Y&ió¶X'?†}iÁ›§?'ñV?Ñ¿?ï"ja!?…×H,ۙ?p¾&þ^?eVfF)>?—ŽOäd?$'"Š˜"?ï¥äj^Ïî?p$¤ùb4?lƒI–(»?[ºxÌÐr|?~þ‰+Ìô¨?lƒéØ [4FGL J1228.7-0318¿î¡âV²ûQ@Mˆã£¨çÀ:`*yPMöÀ<YÊ1çٙ@ê¢îþG@¦^ÛX?Á6šÜ9Ò4?±áàZHJò?ðþ ŸGX"@}Ðãe–¿ä¬ýpÇ?îÙE¶Ãv¿ãñ6É>£¿àTÞ긿åÏó'ªhõ¿íþë}'üAGNbcu3FGL J1228.4-0317NVSS J122900-031758?ï9¯5¶?€Û*¥ãê?\¾7" ­?X
®M')J?ˆ™Í@({?~­d#č?ðÉm?‹‰-¾ô6Ð?S€Ôù)µ?aH¨d±?Œ©)Jzÿ¢?‰ŒY[ñXä?î±¾¼—?‰ûâW'nB?sß©íè™%?d§FE'?¢hi{D?‡y!©š¢?î…
¥Fs?†*‹Wºs?"éá´ ?v\0? Mëk]»Â?€®P·§Û;4FGL J1229.0+0202?ãÊk)«@PwpyåŸÀ6ä^}cØíÀ;HŽyªæÉ@賖ðÇÔ@ë5ó×ӑ?Š Îc*À?¸µmŠœü{@"›y·|°@!¸j¢Ž5¿Ø®gÜÞï¿æ#
%󯐿éêPkR^¿ê‹*k
•¿ëó[ÂHf¿ëŠ
_ÕR­AGNFSRQ3FGL J1229.1+02023C 273?ï¿Ìÿã¯ò?{C™Þ¦?oD£…Ãó?rjOõè}é?pw.KF
Ž?oêd[¦À¯?îßt!'ý?©'ß»ýY?xŸQ?":÷4Íü?ž	"f¼H?¦|ª2s˜?íü‡m†:?¤ÃW¸L?¦º@Wb?ŸnƖÒòÙ?¨¶1HÐ:0?œt7ƒð8Ë?ïõl}ÐH?KCýÏ]?Ci/®?xÔ?BåáKÑ?FäÛömL?@ü3Iót4FGL J1229.7-5304¿Ø0˜ŸÚ·'@#SA|¢À:lT¼ð·À<3uÇ,z@/äbÀ"…@úb>¹y3?·¥ÃH"™U?pN¦þYŒ?»breù7@	2tÔ¾2Ö¿Û¹4i"P¿Ø»b¿ã6쐷rÈ¿ãºI!²o¿Õ;à^d¿çú
­g¬¸AGNbll3FGL J1229.8-5305AT20G J122939-530332?íÞÁg‡ú?¯@ۂ«ií?]+£.e¦?R©…'Â?w?¶Ô]–7¡?¯ÀûÛ/?îPáú¹é&?²ÒÈZ¨ÿL?@P9m?U""*°BÙ?ª° 4‰B?²½Ð¹Ö?í'͵x?™ ÐjT³B?{#îÜ2Í?k‹Ko;Õ?µu'?˜|D¨ÏÐt?ï6 è¤Ç?zQÌãT!-?Xníå^L±?F;½Ê£`?—¥$•'$?z	¨†lÂ4FGL J1230.2+2517?îb/®•ô@U9ý6÷ãÒÀ8C-|:
À;pb·…<ë@Ë[HÐÿ7@ÝBeÖ?›±Ò vX?«Òƒšÿ 4@t/øì@ÓÐÜ{ì`¿Ì8¡1=®¿à‡ÂÀð¿áW_,¶Ap¿àãeË5óØ¿ä+4+€·K¿èjÜí¬@AGNbll3FGL J1230.3+2519ON 246?ïÚ(‹"?we†ìñ"?9‰¢ƒý±?C'ƒòjÐý?qS ±¯?uL?í¡'Ÿ?ï"øÑf	â?ŽÈv¸Ã¥?RÜ'jASß?pÔ:ג?ˆfF¹5]?Šÿç…ÃK?ïZ å…à?'?ÈìÕ|?qñ¡!G;Ê?p̎û–´_??–ýu?~9€Õ*Sà?ïû\	á<r?8ð"³n¯?ø_…×6>ùŝ"æ?ApR'°Å‹?8y<áXF4FGL J1230.8+1223?ßMèKzÊ@RŸag#$ÈÀ8ÎIÚ>¥À;ân×N0@o&ëÒ Ÿ@5Ê¢P!?¤¾ÿô[K?¡íœƒ·b¶?ü84ú³@	=¿©"Ï¿Üj°¢õá¿Ø†3çüÔ¿ãBU&
±¿Þó·‡Á*¿æg;¾G"ÿ¿Ð6äΊAGNrdg3FGL J1230.9+1224M 87?ï½V*òC?r€äWµ?H{>‰`±g??Àå»?~E˜ZÇÜ?qÝ#º|n?ïKRT$
?ŸÁ§®)DT?qB=ö?†©Ôü‹5'?›/…&5€Ó?™O®\l®?îíiá­r£?‹ßˆzez?r«Ý!H?o`l¢œ–B?§ÌˆP£>?ˆæ¸ß†Q?îpyº@]?ÎE©ˆn?•lDëS{d?…g}Fa?œ"ƒÌ©ØÛ?ƒ°aa¢<]4FGL J1230.9+3711?íw*Ðw @SÃXdE#öÀ;kGï'Ú:À<¥}I׺g@:P$/µ$@"¿Z'È?Åáe¶K1¿³J²«¹VÎ?îÓë¤ÿ(j@‡/.kÎ/¿ÑÓ%•|)¿êµ
(¯G¿îÕâ Â?މº¾ØBw¿ïÿèÅPØ¿éièÑæAGNbllWISE J123124.08+371102.2?ï‰"vxµ?œ¶Q­
¯?zð ¡å´ë?'+6Œ"?€?ln÷à?'*ðËâÎ?ï–H9Š?"»S·Öþ³?Y8OlŒ?…¡¶y?‡FðNo÷Ð?·å'ïG·?íwÆ-{?—=tõÚEÃ?'£°ªag¼?uËäÚ+V#?±óC¹Òg9?–1ó§Xm?ïsCÙ°ï¾?‰™Ü粋1?}EúðE?ƒfTˆV¨?"­æ–L
à?|–åüÓت4FGL J1231.5+1421?搸®ÿÿ¢@SÀY!À:YoÒòåÀ<]|Ìy1@ ©.§ˆD³?þ8RÆvq?¼é}1®ù¨¿vª­Nh?½Yۓ"@°ÊnΔÎ?ïڋ1!
<¿èŸݵR]¿ä7sŸ4
N¿Ó¢yg¿ár6é¡꿳ÆóDç›AGNbll3FGL J1231.8+1421GB6 J1231+1421?ïŠ2G;?‹ +•=—Á?QI^µ*†ã?F0ú.\Î?‹JBdÚ ?‹_ü¯ˆä?ï‹ø¤~О?i΅ØMò?F\ÖJ˜?S粃»'?‹™áNs¤?ùA†e˜?íá{«èW?'õÈ0Q?uþ•Ô{?aE?HKö?¯(s›fê\?'ùôÇ=qš?î$u/%´?'=#|?'Û
±ï¨`?oÉÍ•Ù`?©Võ@'º›?Œà™/;Ù¦4FGL J1231.6+6415?åÀ"šl[@J^j¹¦À:"k†`×±À<µ+úYÍÒ@ 0@ºÛ2Á?þƒ†'e n?·8Ô²ÊB.?)˜£i—ïY@sVOiu?ß^ќ•Lƒ¿Úª¶AÅó¿ã²¡r«ï¿Óù5@S­&¿ájQýù•ƒ¿ÄÁK#êÀÔAGNbll3FGL J1231.5+6414MS 1229.2+6430?ï݂Ú1I?e8<7»Å¢?P7æ»âò¾?H§Ù #|?ja2p<"?aš¿uo5?ïv-Ðg¨?'ÙÐ!_ á?Q	'.q?bFh	ß?)µÉñ)º?'÷Õ°r©ã?î1½D8?•Ž™"´–?{ÕÇñ?m{¶qéÍ?©'l9¹?ŠÆëvG3¤?îù&œG?~UP'Ö~Œ?"R'´;9°?jKÀ &l©?–±ã#úc?z<¥Ì&4FGL J1231.7+2847¿æ×1j0Jv@UUüã
®À8—|¼êºÀ;ÒÚý87@^ܯC?ÿFVüfŒ?¡šØÞÓàg?¤:à"BM
@	Dzãí@Û°ºG?ï÷ü@WÞä¿Þi"nå¿àWësÿߏÆ­°}¿à6YSXm¿åRÓº}AGNbll3FGL J1231.7+2847B2 1229+29?ïïf‰):Õ?Y|ñº\?/Mk.´`6?*0Kèú¹?]I@G³ÇÄ?W‹$⮞<?ï§
ªê{G?ƒ­æ¿s4?F>©2?YŽ]_Á÷?"ÛAZÐ{D?'Ì'ïŽÌ.?ﱾѹ?'‡OÓy?pvéa¢?g¾"2_*?˜Ì
͘a?€¦Úk3Ò?ï×Ló±†á?a"VYL…©?KVåËÚä?@›X&P5˜?pî©mÙT?`1R8}x4FGL J1232.5+4821?íøzá®Â@Qm3	AÈÀ:%…—"¤À<†Ó«.í@Xûu·P@_ND0±?¸½gÔûox?³^óUw«³?ø¯²$ªÚ4@m™È"'?²PúŠet¿âÜb¡µÇοãø™]3¸¿çž<á²·ù¿ÜæÿŸ¿ïÿó v,­AGNfsrqGB 1230+486?ï1_\R?? #'ó?k ̺}…>?`ûPɘò?–iÚ}&r?Žþĕ0Y?ïP°«w??'ÞA]×?agu_bb9?kêÊÇ6ú?"½
ž¤Ì?Doƒ½i?횔¢•Ã?•'aýÂ¤?ŒyCcÚ7y?|èÖÁ§?¯8mìàê?'¦f°™?îŒtk•YÔ?‰¡ù&Ñ=?•ê¶¤wÐd?'G!+?˜†»èÜõ&?TÜýyÛÏ4FGL J1232.5-3720¿î<¥dþÝ@@9`ð¸,,À:'…€ÞÀ<M57ð1V@ Ӏñ5?þräùê<?·Óó?"ª—e.Ok?à3
^RÆ¡@ntÊ­7Ü?Òa¤W׿εœ¯x©¿àä/¿á,¿à)ᕱ¿ÉçΰқC¿å_iòâáAGNbcu3FGL J1232.5-3720NVSS J123235-372051?ï7›ÌPÁe?ˆÇG¿vT?bAlÂÙ¿?YGßWeó?–ÄXÝ¥ø?‡ªê¸Ò9Š?"Ó,?"d¤¨ÇÊ?DE+³ääœ?S |ÏËÃ?†ùÌ|æ¿?'Ö§Yœ‡?îÈ³IÔ?'€=¬e?x'ê±8ªï?m\ºFðú?«t¶¤MD?ÆäâŠ?îyÐnqþ?†hªb:'Ý?n#¼ø¿O>?[­òѲ?¦€½I[ë?…ɼÈþ4FGL J1233.1+1703¿íN¾:Ò}«@SÄÝ?á—_À:ûÒvYùÀ< C~ÚÑr@ +ßâSG?öm9ôîT?Öç=¼N${?âX¼$@kªÃˆê@È]Rkˆ¿î™‹âvØ$?ïþT>p©
¿Ý¢¼'ý¡¿Ëvh›ŸÙ¿æä:ýöe¿ðAGNbllRX J1233.0+1701?濫¡­h¯?‡³±%1Rl?pÑæ¢Â?uH6zL¶?|Üɨæ¢?'ˆ9·m?îÒÑö{.?§)#m²?!hÌî×Ó?šä'Ѳ%º?Ê®:?ŸQRg>¡ð?íf'¼í¸Ù?™>[ê0ˆ¿?˜j=QÊÊ?ƒücA©?°¨§‰=ƌ?•õ¡-Á c?ìiŸ•X? !˜]ñe?˜T_KµÞ4?ŽŸ‹iŠ«ö?¶ð(iýµ?œ¯1*°4FGL J1233.6+5027¿Öâóç]@P›'ÿÀ:¼pøŸöÀ<¨~–ÞÔ6@€ïW¼)'@ÑyÚ·q?ÄÈñ¶f.?Ä·©º,?ýˆ¨°Ò@³§<ðK?ï¿ÜŽá¯³¿Ý#¶]ÞØ¿çJ¶!œÁ¿ç´Uý¸}
¿è,œ2¿ïÿÿ)@k*AGNbllTXS 1231+507?îYs?¿Pî?œÂ3DT'	?Ž½¯nés?‰'½}Ã)¦?¢¹`(P"T?˜1ØÔÔp?íUjùޑ•?¬ð]»WÅ"?'>•±Ð¼V?"T­Â%†?°ÅėDJ?©¸ÚvÙ?ììÑiôß³?›»†q`"?–æEÄ—'?‡³½Ú{Û?²ßã?Vܟ?"yYŠ¨,«?ëQ­zÞ*?–î´\F?µw
5?™•ÿL$Åé?²Fh{ô–?"æy"	á`4FGL J1233.7-0144?·‹É#)bÀ@Nhj¹¦À9@'üí&	À<ð'Íó@ðGÙÞX:@a̾Šë?«'Ìx"n?‰ÇcEj\?ÝG¡Ÿw@
î /àÃO¿âù&Çë¿ä,ggfN¿àÊ1|yÎ"¿àî…ÿ³ÔÙ¿àÚßI§ÿ¿ß§†¡ð*JAGNbll3FGL J1233.7-0145NVSS J123341-014426?ïÏêDIM?m 6DwÆ?>êO ã‡?1äã©ãO£?v8ß7o?kî'ýÚ?ïœ`Ð%Ĩ?†ûøe*æ
?G+$ºBå?Vw+"m?‡u"C1µ?…™³²±?ï1|J«ÅM?~²_T¶Á?hÜüë¯l?`Ƭ˜1t?–´×
hÏ?{·jgN
?ïz¹l¿?v7*Ö]]?eé»îa¾ö?R‹ûó r?‹×5Ô¦V?sáƒa…)µ4FGL J1234.0-5735?ámúXe
µ@É°$öYŽÀ9 ø«wèoÀ;¡Ç¯VšA@jª›6Ó?ý1úNX?³…	>Ã	U?Àú¤ÌR©@œZz@	…™0=4"¿ïùw»"€^?ïâY'kÍ®¿ÕpB½ê±º¿Ýa%^ß3'¿Þèê8v¿å=»ýœ£dAGNbcu3FGL J1233.9-5736AT20G J123407-573552?ïe¼É¹Z?™ÁòdiäX?`ðˆßò7P?nS¸}ªÐù?'A7Jʍ»?–woÊ~R?êÇS¤ä²2?Á¥Ñ+g°?|­îz?-<
Ç8€?ÃýDäü^<?Áp•À1•K?ìói,h?Ÿž®t¶?Š0[*wçÛ?'J½Pº†?µ«7l†˜?›OûÌ3{b?ëì
z(û?™ë‡ódj?"ëž_·6?}ýY5ŽP?»¤Ä©à9P?™íݳøÒ4FGL J1234.7-0434?îü ÷©;Å@MWS£ìÀ:ó¥S?ÏÀ<}ÊÞ)@ 9훤`È@|ˆGä?²——`Ú¿Šu¨Î•Ï¶?ÈXŒÞö#@ϗ‰!S?àHLŸëÃ2¿×õp¥.£,¿ãæ~¤ ´¿åy0}¡@'¿Èüªµöœ¿ÞŽ{·AGNbcu3FGL J1234.7-0437NVSS J123444-043623?ïdäñ"é'?˜Yˆ7¶á?T´¦Ÿ¦2?WlH°«'?'³Õc?—;J=7?ï"óóÄé?"߆XnQ??¢/¨?LœÐµÏä?Š<qŠXR?"W›G©Õ?îJyñJú?ö–oõUp?t†ßA£?e¬Fy]Y"?¨Ç…
#ù?N£DIò»?îñ‡á˜7?…i…y§u?`ÁPßÇB?VÿA‰Ø?Ÿ¶øÙ±7?…O
^Ž{á4FGL J1236.3+3858?Èúøaٗi@SoŽ`€sÀ:Ç{ÿTßUÀ<¶=Y&âÃ@íçÈ%É@`¡F6E?½Ša~†Sþ¿¥ ÿ‡?é؋Fð@/UÌ¿îîεY+?ÑW:Ä¢ú¿âé³ÊG¿ÞâʚÃeE¿Ûä×E Æt¿Ð5ÂY¬CÀAGNbll3FGL J1236.6+3901RX J1236.4+3859?ï¿ñédì?z5¡›á¸s?O¿»Or9¶?H·Ç¹EŽ?|~¡_AÓ?wô‰liÁG?אּÐQ(?…OôêNì³??ƒ6¿"û?M;€…b?ƒ×²E¯Ž@?"b
ĝê÷?îáÊAæ{1?'ïyßÈä¬?jf
m@?WôaœS5{? <û?À6?·ÐášõŠ?ïÆa?r$½sŒ¯Þ?jÈׄ©1?Yˆ<¯?‰\G'î•?qZÔwOY4FGL J1236.9-7232?ï¦i‹´ÕÀ#bÀh ÓÀ:~¸–ž=À< ÕÓËò@3òA{ul@Øâý¹÷?È=~æ»?ÂØgµ›Ø¹?ý‡†Œv›h?üy6ð'®?ïÿ–¹‰$¿ç=¾Q‰à¿çw!r–u¿â=n€¿çç]<9A¿ïÿQ÷GËAGNrdgPKS 1234-723?ç¨LãNc?ÁBÒÙôõ?"ó†²=œ¨?'¥ÌY¶C?Ðˤ§vT?Á‡âÑ´ä?Ûø¾£ÚV(?ÌÓ'>? 5ÕÁTl?¤ÏF½¢Ì?áGж¿¦?Ì¡úMK%?èƒ7û?§ög·ÚŠ%?šÿõp?ƒb®%D¡¼?Èýñôr?¥ÌiÊÓûZ?â"ÕT¨'"?¨¹z5Ê(?»‰o8-Ç?¢x8`¢À?ÔغàÑh?«þ®"|9Ì4FGL J1237.0+3019¿îfµª'†>@U`‡~äâmÀ;Ú¶\GÿsÀ<ëCòž@#<Ï8ŒäT?Ѭû¡ ¢?ä9ÓÀÝ?ïÿÐß´0@Œ•¥RÝ?ùl@ûÉ?ïÙÓ`dĦ¿ï;üR?íÐÇÎ`Jÿïì%W¨]'?ïæÑÆ0ÑY¿à¥è'%1AGNbllRX J1237.0+3020?ì朞Ž¤–?Ä0˜öÆB?u3<å4G‡?ˆš›Â?·wç=7–ã?Ã̹Æk¼?ëҏnˆóø?ÆÌe?§¾ÑÕ9+?½é4i&è?µã¥"Íè?½å2ª/n?çԒo‹Ê•?³ëëFÛÿ.?©žËoÞï&?—>	iÛ,#?ÊFeÙâ?´Ãñk?ڞõ²àT?ɳšHb)?PJAï¬î?aµ™–^Ôâ?â¨`Ҙ?ɾø›!`4FGL J1237.8+6256?ïÞf"Mn7@KåâGˆUÀ;¢Qó蚉À=
]Qï@!Ã1Ãq"?ÿ#¶¾mŽ?ÊZˆâ'0𿧓¡2OB?Ùxœÿ§€@A#ݪÀˆ¿ÞGAÝðá¿èðk¢æIv¿æñ?Þ<`Ù¿Ïøö¡]¿Ø´^a4Me¿ÝùÚ·qõAGNbll3FGL J1237.9+62581H 1241+626?ﲧø…Ì?‡—"?7:XOt…a?=£.=Zú?}3~Åу?†ø´A°§"?%º0?‡Ë+Àd¢ì??@7ºK"Û?Y8*ãñ›Ù?†Þ´Ú¿g?†šY•¨àX?îÓÇ<½?•º!Aû×`?k‹γ²·?qbÚ|zT?¬JT‰?"ùéƒcx?ï®,ksYK?rÊez˜ßm?Fp›¹_N?>/äë>‰?ƒ
Ûg"µ%?ríMdbC¨4FGL J1238.1-4541?Ýÿ9‰Â¿@1df±æÀ:¡•ç]rÀ<MI)>¾@â
?#@*k
•?¹ÞÂÿª«Ì?µ b‹l?ùú>¥W<þ@"Ô§äá¿íÝ.^¸<?Êk|»<'¿ã€.Ä8©•¿âÆ®¥šXÜ¿à߸aÛ½+¿ïþE`zîAGNbll3FGL J1238.3-4543PMN J1238-4541?ïé]'$€°?Z)‹¼3®?>'­BŲ=?2§­y³?bÝy3&™Y?WüÙ»–>Æ?ﶼf^¬?€9þ[füÞ?C¢Š%ÂÿZ?R^jävˆ¯?>èD$ï?~b}}+°?ï1ôgŠ²®?~¢U'šª?pF‹\Ïm?eÌ;C:è4?•¯ÐIv`?yGÏß#ê?ïrÞR®5?r.1ë™7¼?j:Xéñ?S ê´'Ë4?Œ¹ê¾8`?pÎɪԬ4FGL J1238.3-1959¿î–'N£|@Eb´·,Q˜À9¨ÔÈCÑÀ<>÷ÂCÜÏ@BÙ¿¤p7@Ǟà*w£?³j·?-"´?­FæÄD½õ?øcì8¢Þ½@
JGB‰½Y¿½:ÙoÈdÞ¿à`ö…,û¿á݇?Nõ\¿á­%!ͅ.¿êöM½øô?¹ðCŸgAGNbll3FGL J1238.2-1958PMN J1238-1959?ï†]ùýò?…#'fê¹Ù?`î÷Œ¬ð–?Uèº%¸(?Š,ݎ.?ƒ"B)>?ï{³€y?Ž5¸W À?Q•uJB¢"?c­¬Œ®X»?Žàmv"Í‹?‹aÜÆmM?î€Þµž?'¶Îؔþç?ŒHT7WaY?‡ÅWIZ©? à	fÑMÈ?ˆ‰ºP¸ø?ïU¯©[?wPe&Kfµ?rqXÒÐ?\'î–Þ#?­¦¾–y!?sõšÝµ˜ 4FGL J1238.5-1201¿ëÈÓ¥Gçd@I[ë[-M@À9{[ùûÚÀ<&=:óñÕ@	T¦ h@@휻	h?³c%ên?°oÁÙԝ&?õ1\#…@µòοT¿ØOãÖԎ¿äþ§°³'¿çõ²JÃÉ¿é2µßËW,¿îAy¢XZ	¿ïÿí )k3AGNfsrq3FGL J1239.1-1158TXS 1235-117?ïð̌?\tÒû`T?;í9®Uº?3$3aÔ Á?Y5³|9?YÙÿå'9z?µú&^?‹•¦ÝÝZ?MëkJõ8±?d'sŸHü?‹›ÌÇ#?‰$é_džŒ?ï/
ëàÁz?|ÞN}òD?qŸ!‰­?cÌÉÙUÁ,?•¶Ú!"eT?yüV1Kw?ïÞ7W¦'?[DaMÃÌ?S¡š9‰;<?E"À6´ì?g÷Û<ªHœ?UWÉl!
^4FGL J1239.4+0728?ÙÏweÖã@@QˆÕ¥¹bÀ:;q¿_üÀÀ<lTdÏ@;݂|œ‰@èÿI Û?ÁfbàtõJ?¿˜á7èύ?öIãxà¼@%U-¥?ïù+
ÊÄ¿ÑÅJâÒG¶¿Ýò
ƒÌ'á¿æŠ=²èö¿çs[wN¿ÐÞÒn¥ÐAGNbll3FGL J1239.4+0727PKS 1236+077?ííP2à¼÷?¢2€¡ó{*?y[úʔš?~9)BÁ?­ÿ}ŽÝî?¡yÔR`f?ï¯71"'?–P-†B*¶?kjJú´A¿?sŸÒo?™üϺ…'‡?"ê>6ä¡*?ìÚë4Òo~?™åm•Z†ñ?'À~,¯?ƒ$Äx+b?´x†Ô©xØ?•óÁ!.ç?íXÙ²Š#?"?÷hôç?¡aWŸv·ê?‡©ÏOHI÷?©
7ç®?‰½"¥ ›4FGL J1239.5+0443?ïǚzVç@PÚôðØDÐÀ7†¸
"'rÀ;q'¬?Ž‹@àðfÚÕy@Ò¢§_U?—ê&yçL«?¿–ˆÌAâ@%|Q£"î@­ï"ã?Ð>ý'¿ázÌ_¶Á¿å%)œ±|¿æŠ ˆK>¿ì«»Û
p¿ðAGNfsrq3FGL J1239.5+0443MG1 J123931+0443?ï¡X±…?…›Ÿl;8?uiñoóÌ?~6˜§̈?yꏂÉÏ?xô֎׬¤?T4©?ªO)m#[?'îgˆvy?•_ªî³½? ûÀڗËV?¤Ü–\íN?ìªxðÿ?¦Äïßwü?¬™•ã×¥¬?ŸÇžÛ	°?¨Åù4™JN?Ÿ"A‰ŽŸ?辶®+¦?xS'x…ø™?s«E;w?ni˜×â†?xý×7qÆ?nÎ5\$P4FGL J1240.1-6846?îjÓ§¦À²-"wú
À9à§7EÀ;çÇc×?í@ËÁPAáÍ@—Yûô؅?½Ñ¾¿?¶ÙþŸ¾ÝÝ?úCŠc›°Ë@ʯ‰ˆ¿à2Æü©3k¿Ý95@S­&¿æj]¡›Æ›¿âˆ?)5®¿äEœAi¬Â¿ïûC"¦%AGNbcuPKS 1236-684?ëÜWSZG?­B6J_?Š†¼ú£Õ¶?€þ%"xÿ?½Ìo¦³?¬
eiùG?âêêW¦?Ç$«9'?t,\m®ß?}†Ùç>)Š?ۉx¹›±?ÇðŽc0ˆ?枋ý'ïÎ?ª)O¸Ÿ?¥Þ·û"?‰:×0¨Z?Ð Œ-ú½t?¨H㜗!?éݵ¯£?ŸÚb€ç3@?¢IIA
??‰pŠ;˜?Ãù~Û¶½á?ž-߃V4FGL J1240.4-2606¿ÅkPG¸rÅ@BXc{ÐZ÷À:Ž£n.²À<;/•Y@€žBöŸ¯@¾¥<e?ÑFÆÞOâ?ÐÍž§ö?ûióžÈ­ƒ@¤­Q'Ñ?îê£aï^G¿æFGhÊ¿à×è‰ÁµB¿ßöÉàß(o¿ïÿùµc#¼¿ätü–¾óÆAGNbcuPMN J1240-2608?ëÖrØà¨?´ž«Í°?¢œ]UÏ ?™—náª<?¾s¾µ'î?±§¤ã²ù?ìÚv‡S~É?®¥MÛËG?•˜¡'2?"n'ñ£?³ê¥¾û¥k?©×Gðb®?é:ˆgnÆt?«GÁ/¡û?±WÃå.œû?š¹"Þ"c?Âiüo­—·?¢ÁGHðq?çL@Mû ˜?¢ÖUÝvö?¬ý'«:?•²‡Âr*?ËÈÿc''Ð? z_0È%u4FGL J1240.4-7148?ì~/©Ìþ²À!ì´®ÈÕÇÀ9y=07FÀ<¤—ú])@ µß5°)?ýì
Š,>L?²'s°Pë*?—¥bzž¶?鍎]ü4™?ýÊâlFOE?ïö¯¿uÌ5?ì|c}ÓÀ\¿åÇ´_¾¿ÖÚ"zx—¿ÔŸ
â@ÒX¿äʤ~z|AGNbcu3FGL J1240.3-71492MASS J12402118-7148578?âÔÓ훢Q?ÆI•)Õ
?ˆZïµÛq­?ì‹Nru
?ٓ€§ßÐ?Æ*üOc+§?èÐ^1Â#þ?ÇZõn1ß?x'?#/?†¦ÑKªP?Ëúu@ƾí?Ç
p|¥à?èTˆç!s?§€#_"?–.Úð7b\?š–óåa?ÍÒ~\å?¦h#°ë\È?ê
m'U÷?¨ý>§Ü´?±Rzí­³? ÓñJ)X@?¾BýÀM?¡õÕx×e4FGL J1241.3+4236¿à…ÏƸqÝ@R˜Äq´xBÀ;²íþu¼À<¸M_.cÁ@ƒÔª;Ó@@Q8¢ý%?Åø\]#¹?Æ´¯Êˆ?Ï"jãù#?ü·»á2?Ó¤ —@¿ØÌÅ@'¿ê¸ÅCk›¿ïùϚ¦ã?ïÆìž#l¿ïÿþBe«+AGNbcuB3 1239+429?ïÔ#hrØ?|¹Æô"•?MsJ؋î?Q«­+ºÅ?r?â—53v?yŬÅßrg?îâ7Ž:Û?¯U]¤u?yú=0E÷¶?ãOF=?:Â'&›?¤VŒþä;?ìö
Àd—?™"X3Õ°?–YzB­?‹C#ö·M·?²¹bž®Jš?"H×/¤B?€ÚK?3Ær¢Wû?M
ÂuC"?XsÃ(C?†Hø·yI?ã¸n˜ð4FGL J1241.5+3439?ïÀ}wéµ@TŒ
Ã7!ÕÀ;'ë£Q©@À<¼tªÌÈ@ ŠõíØ?ÿ5۞÷§l?Äöš;*""¿—»£К?Ԕy^»¢-@|Bÿ*Ø¿ï´4_®t?î©ýýÇA¿åwø_!·¿ÄæËümNb¿ç†´ð75 ¿¿•°ÖÍÏAGNbllRX J1241.6+3440?ïÖ6ÒÛò?˜Ãå~¿ø÷?5$—6I¾Ç?CÐüÆvïb?s #-kn?˜¦÷ÂÔ¦ö?ﰋèÈ«?†?ž¼Î²?=Ú¨í<¦?Nã¾Ü)šÏ?'î0†•5=?…kÆt?î´É=Íá?ˆM@X1Ò?hÆȵÙ?TÁ}9¼•¥?£2ßÁõd°?‡mÔ؂"ÿ?¹´Q?s9Ž+xg?lY.@
?`Mì3º…?ƒ†'éê?plê,4FGL J1241.8-1456¿á	t۟"›@GïAcwžÀ:$ÝpˆÿÀ<D¨ª®•@ 2J*°°?û3	wx¢?Á#øÙÉà?Æpè géô@8Œ{£åM@då²ÌÆ?ïï›2öÍ¿åhrû?»"íe»þ¿Óc҂™Lî¿çÏ÷Å¶¿Å	ä˜ AGNbll3FGL J1241.6-1456RX J1241.8-1455?îžqû¦O×?›MâÚ,›?0­üÚ²:?|Dm:_Ô?¡Ì´ÆdUþ?—ÂnȜaH?î2Bâr?¥ù-
°æï?€dÂs£?"ú¾¾¾º°?¨ÂѨAfó?¢¶b]Jæ?í°]R?›Å?ߍT%?Œ\™œšÏ?€'ulž¤®?³øóˆa'?˜7åÃà÷?ê7îe?¡t°Åàðs? uÔøŸOP?ˆ®?±)?Ã¥®¾—Ý? '3`uŒj4FGL J1241.9+0636?âû­3¨é@QV'è},|À;]Å~ú±âÀ<¹4@€@!#AúÌ9?ÖcÜþô_?âÞJ¹a¶?ïÿwTV™@KƧïž@'™Hæά¿îáóFí$¿à.ŠÂfA}¿ê8¨½ùË3?¬!
ä­š¿Ú'¾1(—¿ðAGNbll3FGL J1241.9+06391ES 1239+069?¬Ö?ilŸXr?jï:€Fî?j-‹AVU?†Y/ÜRøÄ?ŽZÌß?îšþ"!|Ÿ?µrIÞrì?‡)Ê8hê•?­$7~ø,? …¤?Íûe?©gà:ÊÑâ?ìþÅ·š7›? î'*j?'ß+À¹'?ˆxÈþ³í?³Âšx>Ç?Z.?ìp'òA'™?±¨ò#C½«?V†K9×Ù?jüªl?a?¼!ÏA3Ù?±¡?ùY-
4FGL J1242.4-2948?áˆv¬.ǔ@@'-VÀ:ˆ<Ž%ÈÀ<7Cÿ3Qf@ìGÅ•Ï@@OÁß?ÐUŸÚ%zä?Ë9{â#¡?÷	f±@±¨‡s&¿ÀŸRK–¬¿èX;•ØCù¿ëukò—a±¿ïü"J|ûÔ¿ïªH]¼ÉŸ?§c¨¾GhAGNfsrqPKS 1240-294?îá÷Ëó-?Ÿ3S{ω|?'¹<m^6	?'
ÔèqÉ?'#D™#d`?'}2‡Äç?íìLd´L?°­wì†?"A(4¨?™ÎÀe''?²HY'·'?©€£0ց?êÁTBjÐn?£aŠQ?©@cìš~€?–»DS±œ®?½U+ö\=V?šáŸ†'?íÉtÊúÍ?•—<ÖûŠÖ?"3"Ú\@?©xŽZ?©Ï1†f?'yδ4FGL J1242.6+7635¿Þ6‰ë%Ó@DCÿÞr¿À<ºSM"îÀ=2ŠÙã5Å@"o»'!­Ð?ú%kå+hd?Љ
uZ ?­öœ)øæ?ၽí@?ýɸl«¿¤· YfÏ?çïMËdíÀ?Ñö?âÄý¿æÅ!²­<¿ÝÙôhI?ÒÅ0"åˆAGNbll1RXS J124231.4+763419?î·_o?§L'«†ÞÜ?^>PêÁ­|?WÐǧ.Ÿ™?®'œ3û‡?¦ï­€Uè³?î™4fo?¥åï҅ë&?kNéI_Å
?zba<×?¤·ËSò?¤i¶I¦?í^¢¢sh<?–š×'üÖ?ˆ'§ðÆÁ#?ÔØõz?±øµîKæ?"pæb¬4Ê?ìì9ùcþn?¤Â!èƒu?è^ʑÈ?ã"Ýœ?¶a$[Ü"?¤ëú	'4FGL J1242.9+7315¿Óïè
?ôã@Eí?)
»EÀ;.W˜mI¯À<ò],+6@ "q!€XU?ÿ¾ü)±ª? ªõ>¿£ð<àÓa^?às–V;@<¿á¬Ø¼?ïòÒO̲¿éÆ	>˜7¿ÐõDz®Fû¿ÖJªH=†s¿ä6¼ÿŸˆ¿Ï¥~ª*
–AGNbcuS5 1241+73?ï‡B3ª?†dAgáÜ?VíCfsŽ?K\ô-¯'!?‹QÛ*҇/?…€Md0â?ï	³m"¨?–ìP4?Y눫Ÿæ?b¸Hþ•Ë?› "lœ?•Õð÷8úf?îTäQ¼?'ª_~ÇY?sКÔDl?b|éó^Ð?­ž`[±G?ŸÁ2?îfœœü\?ˆ콺.È?'
6EО?kB,:?¥3¨ŽÆ&?‡'Ó¾]`4FGL J1243.0+3950¿Ç+dÕ1>@SKGyBÀ:ÓG:Q5À<–jùs@ûrC>n@ÍÓB1Ó¸?¿‡î`ñ1†?s—'ÝR8?±böð6ß:@tà*?ë—­µ°¿æ´:æ…Û¿é=Ú rfO¿è:ÑÂÕÓ¿ð?ïÿþó…õAGNbcuSDSS J124318.91+395117.7?ïÑU§#NF?vTÌË;·[?t©P¿T€?u8·õ¸h»?J4ìÌ@_?L TìÜÿ?îäjÕûA[?¢¹ I?u`~و6¡?‹ZCó7I"?ž…Š5ÆÒ?"ˆ+i[å?í¡Xr@™D?"– ©ô?µšQ2Vœ?}ëǒ´Jå?®}G©Ö ?¿›€xS?ïGÚm*«ú?….t Œ?‹ñÏÇD?€Ã[Ìç–Ï?'"îM½[?qUÐ¡³4FGL J1243.2+3627?à¦h¿Î•@T œ^o÷àÀ8d çk´"À;w²Ý7~@¸Á¾Ñ·m?úa
 ë2?£k/MöX?®#ÃöÝ@àj¾º»R@oÑ^¬Þ›?ï>S¯­'¿Ô^ßY—K¿Ùß͚ýòµ¿Ñeœ\AŸ]¿Þ"Þð¿ÛWQ`ñAGNbll3FGL J1243.1+3627Ton 116?ì	ŒXF?µM¶Rq?ƒ´x«©ó?½ê×ÙIz?½=)'Ô¶?´©Wä*ú?î"±Ä÷(?°¾ xyª?'Ñ©ÆÙN?£CV¸[?¦ß3ŽÍ á?¥¸·´Ð¦?æðXT"«'?³šIY›?¥ Á'¶à¤?'ÿš;V?Îöne‡™?±//'ÔÍÏ?è–Ùxz"€?±ƒ©?®ë¡iÐ+?'±S?Åé±Ú{9õ?²ò…ïQz‹4FGL J1243.9-0218¿éðÓÎYü@NA	Ö¶[À:C(0 ±¼À<f/çCq@ðÒ]…l;@]°µ??Äv¹Å³þË?ǎ_ê o·@w¥ôïp@au¼o²j¿Ý<û ŸÈ¿çËÿÚ@S¿Ýæ"Cqò¿ß[é€Óô¿æצ
4¿ïós_s-AGNbcu3FGL J1243.9-0217PMN J1243-0218?ï±ÜH?}]dÌ¢¸?XÀÑ¢ÅW?R
…åê½?€·PÞËU`?{p2™Ç?ï¢(7'ù?…á!œø?DRsט"/?U±ÿ¾?†0Êü<x¦?"ÊàLR~›?î Qöh.	?Ž+7'¢*?y"J-­¹?raG#°1ê?¢ÊWU÷iµ?Š«ó*é?ïgœpF®?w0Ÿ´séœ?`·Ø-ßêæ?JY62ê*%?õÌ;,÷?vt^årÑÿ4FGL J1244.2-4956?秊äiˆ@)Ҟ²N©À:‰XÀ<+©­
å@Ê	rðb~@öäÎ?¸¯¤@î?›C‹p*Ö?âª''¥@ÉbŠ
à¿Ì†9•w÷¿ãª3z€Ïž¿çŸÑâ5iÄ¿ßk*ñER¿äóý">5Æ¿á…\€‰}BAGNbcu3FGL J1244.3-4955SUMSS J124422-495422?ï²LP%ç?yÇs½¥V?OŒméËŝ?H%‡+òÕ´?t%YÊU?x-ã_i}?ÈæœÄ?6¢8­m?D´'~»"?Z å›cJ?‡_ƒàã{?w¦¶ªÃ?îÆ\¨f
â?‰<¨p€vd?qSÜݾ}ô?`ÖÏ	*ó?¡o¹ÝçR"?‡6Ãò^Î#?ï0–h«¥¢?w$.5
î?oeå×ø4D?VG¨VM5?–v/ŒEK?uÎO‰µo4FGL J1244.5+1616?ܛÄ-ä6B@SÂ=ÿ?àÀ:žÝõ<ôÀ<'è5Þß@l¦¿òÉ·@¨ _ñØ?»sLþ¶Så¿£1ÁKÂÕ?èIËÆ<Ó@€LÁz?í"ú¾z¿×9ƒ@;Ú¿áMÖ¸ª¿ãýR ^DY¿ÕïW¦°'¿åŒµ_ó°'AGNbll3FGL J1244.1+1615SDSS J124444.35+161621.7?îGð'#Õ?œø‡9h?''Hû^|?wôj¢Õ?¦Ü¤ ·ªü?š¼ÓN¢;?ï:ö[©ù?•—<lD?Zö!ϒôå?i§MÆpø?–ñÜ÷''v?"¹ÊvÿÌ?íUU{H+?–0¼Ù+Jé?Š×)§!|?}OóHu\ô?±úopÚw?'‰Å%"5?í²uªÆM?':/~5'?–«Ž'.ùT?†{lu?©'æÄ<|?Ž¹J<'¢4FGL J1245.1+5709?àx:¥Ý
¦@Mùˆ MÀ:>¢Œ‡b_À<¯è+Íä@‰€Ç»–@x\È_?»KË@ÁÍQ?¬ŠŸM/*?ñ××ârP@³£ùnìG?ïþÂ}¾qÀ¿Ø£k_I'™¿ãŽ.+ŒuÅ¿Ú~(Õ!°¿á©!âRðé¿ïÿâ¾÷!AGNbll3FGL J1244.8+57071RXS J124510.5+571020?ïêY˜´.î?_£[´_ë?@Î*K¯\?7¢M‡a/?arÜÃþ(?[®Ào^ð¥?сÞ?ˆÊ¹÷½¯?Mgژ·E?^°€†›?ˆEÞð®?†äˆÊؐU?ï#µC÷¦?€Uý"ú8­?iìcYÖ?Z.P1	8N?˜KËçcy?~¹yõÛ?ïnZ '?rÐĪ©"?~îH= ¬?eH'¢Bö?…[‡‰$?kDgƒ¹±4FGL J1245.8+0232¿Ù Ô¢j^Õ@PX4Á¨¬\À:ÒùXF3À<°·ŠEhÀ@‰Y"Eò¨@cIÙgåÂ?ÇҁÀá²?à©=EÛ¬d@U$¿ÒéG@-Äq3žé¿ïâ^¯c?ïEmþ
\z¿Ú!Ïþ°t§¿åÞ¯6'¿í8´FÄ	°¿ïýðƧÞAGNbllNVSS J124533+022825?Ûb|
'û?ùnƒÂ.?ß%þ",AÏ?Ŝê%{ÔØ?µÞº¯o?¬±jP^?å/jZ¹•?Ì^ð­tJ?Í%VÔg?É9áGô¿š?¼:œr?²ØĂ½È?ÜÈMÞ£Q?ºÍ/.¨—?Ú¨EDJ?»"îàëwª?ÁÚ<:%"?¡Ì>–—]?àý6AÛVU?²£¤˜1Ž?Ø.ã1Æ?³YZF¼3?·ZÁ(†?? €zÅ&N4FGL J1246.3+0112¿" &ƒOêÊ@Pʽf'À;0íæ²QÀ<¦¦3
@ºþ‰³G–?ý*þE뜜?מքÜs3?ÎhìƒK?öz¬(©l@o…r›(¿æhŒEô¿æ¸Ã*Œœ¿ä÷'î\i¿Ä‹í¬vì¿åïw‡ R¿ïù}š_'7AGNbllPMN J1246+0113?ïµÈñQþ?~㶃‰ñt?HE"¿Õ?B¶	AƖ\?	¤k_'õ?}õ'ˆn_?ïŒK$ D?‰• ÌËCp?DÕ -캂?]á('Y ?‹Ÿß3ù#?ˆOÉ&æ'?î9"^õíÇ?'éɺF	À?vþÉ•  ?he¯ˆÈ?©†àðN~?'x—nc?îÜÝ@çÉ?†ÓhLܵ?]_ǚÖËÆ?SbN~"?¡G/ßÍ"?†1)(p)4FGL J1246.7-2548?ïþ¦b™—@B‡jƒ+™À7]M•µ‹À;>Ð}[ur@õ@Lz@¶ŸÜ©¹¢?"i†<«¾?¾îܗ8@'w,¶Ap
@ð‰JìãC¿Ê,jÈÌ¿àf¤^ïy ¿ä؅½™©	¿åÿdd-§¿çȽ¼
¸¿ï(	3…iAGNfsrq3FGL J1246.7-2547PKS 1244-255?ïË=!n?v>ŽJÚì?IýÕ (Aò?Pä1Xä?w!´½Cí­?t™!½â™?íš@PB>?´útR
`Ñ?–¶ÖЗ·I?¦ãQ¾È?«"'Ð?«û˜ڑ«?îÌa¬?•&ñe
?'æËo°ð?'QͬT?"]ÖHlِ?Œ"C8³0?înî—I?˜°¹&†Ë?'ÅŸ¶Y:?ŠæÝîikâ?ž'y³Üt?'[îGï4FGL J1247.0+4421?ïРjTmÒ@R0
ú/§À:j1ί%À<}ËÆ<Ó@ T¸?ú+Ì¢¢&?Ââg=Ñdz?ÂsLhckµ@óþº…¢l@šˆÙ-m¿í3e"¤7¿È[QIô•¿¿Ø¬@»1ý¿ÐÑÑCſܨݤ‹e#¿âüê×yÎùAGNbll3FGL J1247.0+4421RX J1246.9+4423?ïáÀßýÙ¡?h² ­Ã?@+ҙiËn?:š98êÔ?j4+[Ëêå?g†®¯z?ï™lD®u?ŠÝm•£Þ?J—#W"þ?Xçyz7?‡û|žêlw?‰IÑ|ir?îǒÙU?‡ŸÄm+ìÍ?nzxqŽ¦…?\ϟ˜Z'?¡Ÿ*㖳û?…¾üä öq?îïVa9—N?'_ƒãXç?qñüýEŸ?b6ÿC5Œ?˜´™{µÕ?€ìC'êva4FGL J1248.3+5820¿×'æ{ì×Ò@McáÁP—ÈÀ7²ÂFbÀ;QDy¬"H@#'0iK?üù!ÚE[T?"ZýU­º?§]®1S@lë5m @²ŒI¥¿ºOOŸx+¿Ü[é B*G¿Ý­2=>ú½¿ÙŸÕ]jo¿áGßÝË¢«¿à;‹ÇHÿAGNbll3FGL J1248.2+5820PG 1246+586?ïÅÁl֍5?ƒå,uÞà?7<Nëü¦Ô?B­¯°tõ
?{«"¥ù›F?'—=Ì{é?îîÐôê ? Àœ·	£?mˆ+á¬í'?~«T‹êŸ?žtÛæˆn7?§y†ØÄ?ï/I#'»–?ˆÕ7{",Î?wåuº2x?y)
eˆõ?"~ZÚ‰?"ñ·'¦¥?©·?Š‰$æ»X?rœ²@Œ''?eŸSþeC?šgþº¹ß1?‰Ð*A¹ë4FGL J1248.7+5127¿Á-BÔ÷ú´@Pj:ÀÆ.MÀ:çÓƼ"À<Ö35·qò@ýV"U@sˆ€l¡ê?ÀOBßN…?  ÜÄf¢?Ðσ@;ÚL@ô%ä–.?ïúKUhè!¿æӀ y\¸¿Ømû:ôG»¿áTBý«'ê¿ä¬œ«¿Ð7h!&–BAGNbll3FGL J1248.0+5130RX J1248.4+5128?•™p?Ò·øhY?UŒRÄÚ'?Om®kF¥?ŒøÉ0Á?n&‰€µ?ïs·'Ýhå?Ž»Dx«w?KŸ†{XG@?[Æê­ˆU?¬px!/?¢|,•q?î9šÐ¿b?®'<FÅ?tàìäÀÕb?c…¤
–Å?©Ó(¶[ï?•Š¦©Fÿ?ï.ú¡®q?zŒ8fáï?x¼ñÄ"?a·emG|?"O/ŠØ?xCö?¼4FGL J1248.9+4840¿¬äbÄ!@Qý`éNäÀ:½´ò»sßÀ<Ã9W9¢¹@=x±"ø@2™åﳂ?ÂxÛ^?«
®e?çˆäu_þm@)Ùçg'Æ¿åfH3ux¿ãn¯«SÖA¿æýh@[9â¿áV¨ž[¿ïΗÝ×·¿ï׌CoÁYAGNbcu87GB 124632.9+485605?ï­8BUô?Ÿb¸ÊÿÑ?`*?z¨"'=sÈ?€°ì3Ã^?™` —æy?ﶀ€7o?'6æ>òéR?>}%âö§?QW·‹/0?k÷Xõ&þ? º‹k ?ïÛF;¯K?‡h¢Ù&?p&X‰š?b^Á«ØOB?™û)¯ï?…½VsÂt?ïۅÅîÍÆ?[–ð²ñ?XI¹Ì1U{?Iz=–R½?hU]+»?TU–´™4FGL J1249.2-2809?ç8˜V'L¸@A\ÂzcÀ9óšw+À<J–6—l@4žm=ñ@/»õäô?¶ˆWQölÙ?¦
L46?ðÐÄ©Ü¡@!åÆüÌ¿âÚ%æC–X¿Ûhfç¿å&ýšÊò¿ÕŠJWu¿ã-ª}l'O¿áž¨âŒÒŒAGNbcu3FGL J1249.1-2808NVSS J124919-280833?'cò9?y·£˜9à°?[þք¸Êˆ?Lä7TøÕ?‰YÀÖlX–?x'ö:ÌØY?ï˜^°
¼?‡OD'ž&™?Nw3'›t?\fõáò/?ˆàŌ—H?…îÅ7-â?î¼s¢Œo-?…v¸•±ˆ?qɲ8´B?^€C½(Fö?¡ÿ£àñö¸?ƒgú-ï´	?îúMθ=?;ÄMžã?|Ï쾛V?d`»Š^"å?™'R-ȧ'?{ž]Lt¡4FGL J1249.3-0545?íëçH'Ú§@L"V!uÀ9ìfknããÀ<)ñʳ@°5;Ì	?þ°ÆÜÈÃS?Àßäׅ?¿|F¢{Àk?üðÁo¡y@
óÍ]ìDa?±–!êá_׿҃Û!#f7¿ázá}]ù°¿ÝèèŒEô¿àáMø±W&¿èååvø…AGNbcu3FGL J1249.5-0546GALEXASC J124919.46-054539.7?ïîŒwéÐ?QNÒ,¸pT?<'½YµòY?5*!bú%?[ Õòz?Mÿ@©úy?ïŸù"&ÂÒ?†_jé¥mä?HOdŽ°?W\¯­–O?†yª'£?"éUsw3?ï&GCì^?~±7…ÓÔ?h©‰¾x'?\]¼N?˜!æz*¥??{t£´ù!Ç?ïŠ/4'?|;J»š¥?ph_&Ð?X{v,ÿ?˜N`¦7•?{5L´ëö¶4FGL J1249.8+3707?ãñ—"h@Sÿ|E˼,À:5áŠëÀ<ZÝÌÏQ@ —øo'ßì?ú¤Ò—çè²?¾š½°û
"?»ÊkH£\ç?ùkøáþ9@v[»¹f?í÷G"êp¿ål­byFé¿Òv2â*'
¿ÆŸiýŸ¨|¿á¨[ý¿Ü'ÁM'AGNbll3FGL J1249.7+37052MASS J12494675+3707474?ïé†Éÿ·Ü?fbNìÿ`?1_×™(±?%¾Xü­?dM;ôýr?eÖt4ƒ9?諸¡%¥ç?‡A<˜?Euþö¨S8?VÈ0®'"?ƒù÷Ç,?…÷BJ¤?îóÓMäøû?†™ˆ©o/¸?d'GÿT?RS,U9U¹?žõMC|"?…š%Y¸V?ï$#<Sì¸?€
–£Î®?ko&G×?X+ýE1?˜6睟ò?~'³ZáB4FGL J1250.6+0217?åD,ÊZÎû@PJ%®æ1ùÀ:7Faä ¦À<[DÐêh¿@Ÿ0'ü?ÿéki¦X?½e?½I?µô'žUk?øՐÀ­Ú@¦û˽Ù?Ú¿†ÞV&?ß¡B‡N¿äƒõ¶6ˆ¿Ù­K6_¿åÍF¿×ñĿُ­‡'›AGNbll3FGL J1250.5+0217PKS 1247+025?îÎ~ªê?'ŽïY"ï?}n'Æ(Ï?pTL¹ý-c?žáŠÅq?'V9
 Xâ?ïÙ Y?šÎ"ºàî¸?pé0ÌÊÝ?~ØA™Êt?˜ã ™lò?•€ÿPÆ¢?íŠÿ7+ï£?•>'휆¸?…q1Q	û?r"ÖÀT?±Ø vaœ?'°‹† ë?ëý¬Ï|Ñ4?—67ÿ·Än?¯—e¸à/?'§N/­ª>?°F槩pÇ?‹èûÔ}€4FGL J1250.8+3117?Ü8¸`â¡@UuÎ1PÚäÀ:½^¿¨÷ÛÀ<³ùJ÷@½ënM'@dà?p?ň#û\Ø?ÀÇ`âÃÚ?ú4Q%Œƒ@—멱¿«?ïéæ]Â}é¿Êp¡Mm¿àÅîÁ껿çoñ)£g¿Ø§9ª€¿ïÿãzŽ;˜AGNbcuNVSS J125051+311706?î|šgIî(?¹/mVõ6?i‹%2bJü?‹¾RA™¦?¦§8:øÕ?·D­©#?ï"Ú3"í?Þ_`¾<?H\ñõ­}/?V+ÀHËk¿?‰ƒ£üÃí?Œø`Ìÿ©é?îŠñ:v-T?ŒŽNÐg?sÔtgò?h‹Æî¹8î?¤ÖkŠI?Š'ÎZx;i?ï(yf|˜?€ÖíŸ^À×?{M6.Þ?m}t§Ë~?"
Œbá??{ðÓ Àé¹4FGL J1251.2+1039?ÖÚjŽXÉ@Raž­ÕÁÀ:È_Ñ÷®ùÀ<Ûž ç×@å•á"@CLŠÅÁ?ÊC#–21?³Øj9ڗ;?êÿ'>‰(@y	ڛ?ÌöÄŸä¿éØS³Ü:ÿ¿Õ—zEˆÓ¿ßѾmþ¿äóUÝ­Ô¿ãØr¥®AGNbll3FGL J1251.3+10411RXS J125117.4+103914?î«_¿ÅÇ?±]‹øº"È?-Ñyc?­âŸbì'? þ¥JêÛ?£ÚzÄÌâ?ï›ñ­Þ%?‡×1ƒòßm?A6(êõá	?Pý=¨bËV?‡ð1ùÇ=å?†ñ>w€?îƒÝdã?Ž ÞÈ[Oú?hkø~ .ø?YÍáHüØ?¦;j0Ìx?ŒéEœƒ'ë?ï7^A¦‰?váŒÓܧ?ef§bÊØ?PèöÖ7³?–dþÕ>?v8ax£¼4FGL J1251.3-0201?Ñ®¹ÀšSB@Nl)Ür\À9çÆaxÀÜÀ< ªÍÛÁ@Wš©+½?ÿ5}?Æ¿m?·íå᛻Þ?Ãð\žçaN@
–Õ"õÎ@Ú\`ˆ×?îÃRЇlp?ÀÁûxö¿àÖ8¡1=¿ãh&à>™™¿è	 B*Fû¿Ü.]Á&PwAGNbcu3FGL J1251.0-0203TXS 1248-017?ï°Q͂È?z±:?¿?g\¬'?k¾ÞÃ?|1ɋEà?sÅܺµˆ?ï¡>bYý©?ƒÎ°±Æ&Í?GœËbؼç?ZOäà÷Õ?†6š³S
?'s&#P?î•
a²&ú?OËôK?Š%¡}–9?"ñ¤+R:i? %Á…xý?"1íé˜l?ïu—×Fm?w7ŽXc?hNZ67»p?W`q^%Ýd?Œ†s¬ v?uRj·1 4FGL J1251.3-1719?К+¸žC@FÆ~¿"ÀÀ:ƒ½‹ç)À<0'½,EÙ@Œ½T´¸.@Rå=Ì?Åi ÕãvÝ¿¯C²¡To?æÈa-A'?ý"ˆ'ðਿã)ò­1&¿çôáSlŽŸ¿èÖ¨]¬®t¿ïÿþó…õ?ïÿ¬ž5¿¿ïÿ±%§YvAGNfsrqPMN J1251-1717?ïÙu©¬Û4?wþ4M¸?[Än̝­Ê?bי÷àš.?h¨ìÕõJ?r'–ÏB!­?î©ü"4È?²8JžÃš?'Ý4ÐÂo(?¦û€ÈñL÷? ¨êˆ'âq?¥*ôÔ0n"?ìnÕà/–'?üµ¬) ž?—UOÐÜ®Š?Œ`¬"6¼_?¶³ý
L Q?—}ó{_½t?ï§fz›Vy?… Z—Of2?=›9Žßa¶?P2èICä%?…9‡Œ³f:?…cv+4FGL J1253.2+5301¿ïRCwàœ@Pö¾7ޔÀ8¢}À;`F'µ@F‰!|?þæ™&­ó?äè!'ö?¶Ža¯Ž@}4ßݵ@¨ªƒ¡¶¿´wù
îE˜¿ÓFšDšd¿àíA·Zu¿àVƒ?4{¿ä\¼>4C)¿äCëGWLAGNbll3FGL J1253.2+5300S4 1250+53?ïØ+ä¢Û?nø¹¤×8?Að»i:5?HŸÔ=¨U?q«öAÐËÀ?låÌç¡"?î%h=éƒx?­hr®C'ˆ?Œ"³¥'? "Šæ‰V?¦"v¡:ß?¦:}Hl·'?î¯è·Ýõ?•
zB"	Î?‹jIðýT©?ˆ9´SC7<?œMÄÝvø?%E)P?ì™g}¤e©?Ÿ­_=§N?œ—ÞUFT[?‹²›•Öâ?´Ì}‹=¥?›nH?r—4FGL J1253.5-3934¿Ëÿ8ÔKµû@7M‡ø‡eºÀ;Oô!¥l6À<­qGÏ¢@"RüÎÈ$œ?õ»
7 '¾?×(ª.'?ÞBãÈÂý@\ÝF—"@hU¥ÎÜ¿ääáÞ?¿ð?ð?Û襁6¿·d^ -¿æºÀZ΂¯AGNbll1RXS J125341.2-393200?îÃOé‡4?®_Ïr}P?pšÑÑÀ<?o<ĕ>b?¡É­TÆ?­ï†yˆ¼i?ïa qÀ?–ayå«Q¸?[h·ä³?uAIÒ4"…?'%fcnðË?"²͐?놉@EŸ?§š½­¼!Ë?ƒg뽞¢?u8ôôÑÍ?Àµd€÷¡?§3ŽmAÙ?î-'zà>H?žõ}	»?JÊqjI
‰?KÍHЀѣ?¬»®ŒR÷X?ž/7Ö\4FGL J1253.8+0327¿îMv
"z@P"3œ¾àÀ9vZT	lÀ<á¦x¥-@—˜épq'?þ¨S¦pA±?²\[J©q~?²ï'ó²ê£@ºÆ:"‰@ÂÂ¥V'1?ïæfÁ«¨¿Þlâ×P3¿ØÙL!–¨£¿âñµºa¿àajþütÛ¿ãIsÔ
3AGNbll3FGL J1253.7+0327MG1 J125348+0326?ïˆaªk?H`e.Ï?W¸¶>aî?LŒ§é9½?‹P͙ß?}¿ßWÛ?ï†g=??—†rþÌ?hì³ÉO]?rÖ¤ãÀQ9?›§™îv5?•;ì7MP?îhivO…–?gu²ÁÊV?z¨ƒ+`X?rûӝ3[?¦$dê¢:–?‹+EAûÅ?ëÏ)gûo?Ezz¾? ~(.Xhš?ˆg…{}õ]?¹G¢ý"ð>?™ý}t…_4FGL J1253.8+6242¿ïì­îg§@K5ܜM©À:YÜë(À<Ÿ!ÿ.Hé@ì˕j5?ÿRþûB0?³Dç­†?—qd¤ÍÝÍ?ä
*àÔ@´@»ù¨M?ï§0ü!N.¿â®¡Óú¾x¿àý¢È6¿Øó"
3`¿ä¾‡Å[¿C¿Ú†«ë«µ%AGNbll3FGL J1254.1+62401RXS J125400.1+624303?ïè½_¥~é?f4Iy*?:	«
e?8vìPoÿþ?dŸ%kY?dH
?敏 ß?"Y?œt3?Cj¶Sˆ˜?S³™Nø?"i"±‡?ƒ
ªâo¥8?ï-õ&rjT?€>Rƒ›ÀQ?dü¡£†…?SóÉ^½8?—¡Ç^DÀ?	߉·ÿa?ïºÞ Òv?ew—ó¨Õ?^ûéì«?Fj" îÄ.?zÒ(ÿ¿/?c]†çÚ4FGL J1253.8+2929¿í¹k½NÃ@Uä‡Tów\À;¦JœÜDÀ<èdØǬÒ@ —aºH9?ô‡™Sù?à?…¡•ž?ÕÜ%³î¯?ó¬õ–ðqî@ Ü&$?ïúÁ.ˆÿ¿ïÌ{n5gÁ?è¨+b"Y–¿ÎfÆÞvB|¿áŸÂ¨†œ¿à×QÄòAGNbcuFIRST J125405.0+292708?î†ßEœò²?©ÑÄÁ[d4?h-È=h™?e÷˜?¦ÈɬþV?©N[Ç^?î»âiD¡?³Õ¢2y?e,Š?w¶i	s‰×?¢ïà=ªý?³X>‡ý°»?ëôdG%3?¥'Ë™œEÑ?†vƒž±Ê?x"XÔÔf?½Ž
Vâ't?¤Þò¤Hêƒ?îZ¹o²?œ—J»f¯?N;"¸m±?OãÀ—Ê(N?­ñgîûó ?œ"¾>Ë4FGL J1254.2-2205¿â{¸²…ñ@DcÖ¶Zš€À:I}.ÿÇÌÀ<HéH-–;@g:<fã@	ýñ7?DZÓ!O°í?Èðužg´š?ÿ|卍ó@
Ÿ˜^†;?íŸ9Q´~¿Ý¯Òò䏿â0"刿àµ{!	¿åI¾ RÔ¿ïÒÁ££Þ—AGNbcu3FGL J1254.1-2203NVSS J125422-220413?îæË="('?"'—f""à?jº®Ït`¶?d×þ_âL?ŸÏBsŒo?'ºµì"ð?ï\|œ-oæ?Bïd?U"P"%?`¦'ór×g?"+HɄ?‹˜}²ì£ã?íäÊf"C7?–Tˑ˜I?'E¬Zí¢?u¿@T?­!îvu"?"1¯ÂÌã›?í á#‹™O?Žkò&6È?…"ú 9*?kbèyŒ1?°@¦D_.j?DŸãLð'4FGL J1254.5+2210¿ïO𺁊s@U@'(bõ™À9ÊôWÀ<UùK°Øz@¢v Ë@£iüóÜ?¶¢`<«¬í?¯«þöë"H?õUŒ·^¦@…Í»Š/C¿Î·_}>@¿æÕïUÑ¿Ùý"$½O¿Û…íÀ7h!¿çO;Ý%àd¿æp÷б^AGNbll3FGL J1254.5+2210TXS 1252+224?ïæØ¢3Ý"?Y ÁÔ`?8Cf|
z?-dJî?fûßS\2?W¼^$XФ?ï"]Щb?‰k&Ï]îP?N"ù™ä…?^"hÌ9oè?ˆÿO'7e¿?‡ù°³¹ÉŸ?ï8úp"±\?~U¶O™ Ý?i1"T7d?iU&R7Œ$?•º£ñ9?zH¡/ª;A?ï%×¢}.?~9¼."ºF?|aåEY?eŸ5*
÷Ô?"W¬É·Ñ?yï$ôƒ(#4FGL J1254.9-7141¿¦vÃTù¸…À!¥{"ÛœsÀ9û<š»ÉÀ<³"&jÎ@l·2[ÇÒ@>öÞN«?¿j%®(ó?Ã?áD‡@làÓêÎ@®qLÉ\U?ïòr®sEr¿ÜC¬ýúl¿è$dIU´¿å{ඎœæ¿êˆè""©¿ß'ÿùtöAGNbcuPKS 1251-71?î0M{'±?²–¥Ü¯Ê?†Õ:[Ü?ªù+Ýן?§EáaƒÝí?¨ÀFßL:?î)'t?°qÚ¸˜O?B+/Úm©?^™š¥fJ?­zxdþ?°aˆ÷ŸVà?í_†_Ü®?š³«Mž`?‹->!«?z¯"ÌŸ?³çc¥<ö¿?—ƒñÈ£²Ò?ïzÍ<.»Ë?t¸¹lש?Zì?{oë?EIR"`.R?ï)ã*?t›l)>V4FGL J1254.9-4426¿Ú3Àá0@2lYtæ[êÀ:DN®¹¼OÀ<;hë{ä}@vîªíÿÍ@Uçþz¿?¼ýòÆ¿‰B
ø'´‰?ʎ"õ"@ƒái\æ?ïèÝ¿cW¾¿á	Ê^ˆv‡¿æ`Ÿ¨žð¿åqž½c£¿Ö5ÿ€Ô%Ý¿ïÿúVrÓ\AGNbll3FGL J1254.9-4423PKS 1252-441?ïþ¾Î ?"¼È€Ïq
?x½•"ÀÀ?pk€@ÛÝs?—þþB݋Ñ?'ñýÅeì?ï9_Oÿ)?•+ǵ"?T†ã˜ÿÞn?_Òr,ئ?—‹§ÆŠÞ?"'Ý‹)‹Ú?í[3uˆ?—"á?¢ÊSY ž?z´°?³Íëß²?"8'X9ó?îqÌÃ?†Ré›ÕÒ?{ß°
€Ý?iÕ3¾ôGè?¥r>_Ø=?"`Óm7Ç4FGL J1254.9+1138¿ÅŠ,Uë¼I@RŸ÷ÎÙ‡À9ýpƒöš&À<;á~4¹E@…6»©@õ–AöD•?¿Rj,d¸?ÊÐfŠM¡?ÿÀÑìÇ>@
©ØÎã¨[?ÙO³œz¿ã³ü†Î»º¿ëò…žeh¿è¹F¨Zý}¿à×Ë~3Ó¿ïÿœ,ñВAGNfsrqON 187?ï±"mùIH?"÷DAä:ª?zۊ¤UþÞ?~|½:ÄVP?i&|¾
¹§?pªàÚmç¸?ï1Vˆq\?˜ÁF©±x?j
cô&Fô?zå§Õf#?–œÈ°m¨?•TVåº?îò !'?—² Õ¯Æ?•»¬¾Š©î?ŽÇs†HGÑ?£¢ÿž©ü?‹²@	¸€¥?îÜÕí^‰?‰o¨Àa.ý?'
q䄎|?"MÙ0Dÿ?'Zì}Ï 2?xÇÿ‡&%4FGL J1256.1-5919¿×
ÀÒÇ@_0ÓÊÀ9Ç\ŸTÀ;Ï©mL3µ@ uxj…@újÊy5v?¸Í¡Þây¿™4YªÓ?â#Aî·Ù @B2<h;(¿ï¼IýzÂ?î—È©Q'¿æµLG×/&¿ÞyÀGƒL¿Ý€&Ö@¿ÞêiÀ¸íGAGNbcu3FGL J1256.1-5919PMN J1256-5919?ëaˆˆ›‡•?²Æxøóß?yjn\† À?rm!©üÉg?Á®Šj­°£?±µð$z«?éë`…wM?Áb•Paà?d"«´Á?uùf´hõ?ÈMŸ;OÊ?Á/{ºíæü?çxTäl­?­ZI9Í\–?™äiîÑ?'ƒŽ=?ÎâM<v?ªûß
E‰V?ìós³Sá?—Éã‡""?6çÜÙ¼ˆ?vøw½vU?»á‡fÊ)g?–²ä¯	f4FGL J1256.1-0547¿íðóô³›@Lˆ'ùD$À5…¼ÇœdÀ:}2ñÄÓÚ@"¿/üÈ@'d¼B;?y@X¿	?²Û''ãB@0­ÇGQÎ)@$ ?ö¶¿ËDYv=ôØ¿áVƶ2W¿å='AŽ@¿äsçŽ2׿é=Η¨(¿è·_èã«AGNFSRQ3FGL J1256.1-05473C 279?í¶îÓK"i?®‹©<@A?a"?úß?ošB¬?±¿¥C£…¼?­øêwƒÄ?íðìhw\G?¹öî語?'æ&Ðj-`?¨óŽ½o‹?§þ&U$ö?³ûèáSº²?ìŽD#^˜?«Mð<Â<?•<cXÎSç?'I,±ƒ:?¶>Æ׫?©8'-té?ïsBkÉÒ?'™ð7a?m~áN2Û?t̯8¡@f?‹ëE€¹þá?‹Ó<%$÷4FGL J1256.2-1146¿ïêO¦í{@IŠ<æÁÀ9r‹ò)ôÀ<øð@€-.â@§?þD
Öó—<?¯@ÄkTa×?›×Ù½˜sÌ?ì'Õ ™@cO•Gû¿ãèÔÀ6;{¿áKû¡K"©¿Ø}ŠDg
*¿à‹ã˜Á,†¿Ú…뜛¬™¿á¥sŒ¿–ƒAGNbll3FGL J1256.3-1146PMN J1256-1146?îËçP®h?•i¬ÇÇ³?pq;×?cçºOËǯ?¡>œÑ7¨'?"*e=`4é?ïþg"9í?—Y÷<õùG?cW9È5c&?oJåÍf?š5KÖr	?•º}•ë\?ëڐ	C
?¢'´Ž‡‹—?'øW5™/]?'°Ðª}Å?¼­iè[¼? Å+$—K?ì?…Q-U?Ÿ·k·]Ù¢?i¼hz??yNê	ù•?ºéV?Á
MY3ñ4FGL J1257.2+3646¿ïRX¦EŠµ@TçÿX:TÀ9à?d‡À<gñBÍÚê@1ÆöI?þ¨™Fƒ?·›"™ÐK2?¹v´è)ŸŒ@Ìø×Òª@
ö8#¿çtØïð¾D¿×šƒT]Ð¿à¾V<"¿Ú«
š¸¨~¿æ~VG4qø¿ápq·Ó@"AGNbll3FGL J1256.9+3649RX J1257.3+3647?ïñ™,æQ0?Lülæ	Ï?2V{[N.â?*ÀÔ¨ï'?X8\Š@?JV+"ó‹?ï™4e6²'?ˆž
ù^ªj?J§Hã£û?`@?Q°ò?ˆr$/=?‡2Wܦ,?ïBò¦¾Éc?zR²Ôšð›?föÌñêM¬?[9ÊyƒñB?"Âщé‰ç?x%Ö"¶ÌÅ?ïWè¤;JÄ?xªéKáÄ?s\RxC?]²)¦ò(?+ÖÚoV«?u¼ï]·§4FGL J1257.6+2413¿æTiõÎ4@U±Eà´áÀ;̀üê¡ÊÀ<Ûû()êµ@"1Žw&¨
?ùb¡ Ï?Ó¶…">C]?²Ýí§^Ô?àyt*tGÐ?û¢Ü)T?Î<©Ôz@8¿í¤u•®RŽ?ªá¡½våÝ¿Ú
÷À@wi¿zQ–åNË¿á\ǶãV|AGNbll1ES 1255+244?ìÏÿ¸õ¤F?ºÜ!Šã2ð?Wš€2Á¢?Q€Mç]Ù?¹!˜7Š†Ì?ºÏ+Näk­?îHžÑ›?µZ$K'Ý+?qXïã½–?€y8p® ?©KƅΤ?´Ó~Œð?ìýÜCõë"?›‹p]ñÎ?t¢HTˆç¾?f±9¸Ø?¶Æù[Ü?šøŸc'ù?ê¨â†¤x¹?«FkP8Š?gœrƒ:Ѻ?f‰"ò?Äþa1Ô?«>;ù
M4FGL J1257.8+3228¿Ð'æ•Sll@UwîN&ÕÀ98dUêî À<	*	¾Å£@|%ÉX@À«;'?«Û¡&ŀ?ºS*tr×@µ›Á'@'ãçp'?ïÿîbHÊt¿áû–ä³s_¿äDÄU/¿äÚ
\ßÔç¿ê9yh¡ª	¿éN‰€Fâ=AGNfsrq3FGL J1258.1+3233ON 393?ﳶ=–ÿ?€NðL8Ô?PîÜñÁ|y?LÒñ!ƒ¿?€ô•b"?~" r7e;?ï ³¾¡,Ç?ˆHt¹ð'´?I"íÂ‹'?]4zø@‡?†9Á~Ø¥P?‡r†!û¹?î~‰ÔQF?'½±Žáú?‡÷Ì¿ˆ&?€N³#A²ª?¢o´öI•?Ž5¼‰½5Ö?ïÛpz)?]æñ±×?R{	L…°ª?C‹àãØ1?kRwߞþ"?YÈÿî'/ù4FGL J1258.3+6121¿ß.ã"ôÐ2@K߆
¢À;K›	bÀ<ò"Ì@"öàqšL?ýwœiW²n?ÇÉey¬iU?ÅÚyMBÔ?û$Éþ¼3"@§éÙM
Ð?í
z<@Œ?ìŽù,§'ø¿Èêû÷\ÃO¿Þêz\½p8¿äQÁÞÝ£¿åé÷ 54AGNbll3FGL J1258.0+6120NVSS J125820+612049?îï7iÔ,?¡A›;t?'ï¤î9'?Ÿ¤Ò]·E?˜¡@ehí´?
݁ëÞ?îñâe½8?›sý•Fˆ?qMó†¬u0?zlº†úþô?p6zÝ;³?—dƒ(aÞ?íåÛZ§çæ?'pÀ‹Ç!5?ôA¢›Æ?q%Ô?u¡?­£ÉMM.*?ÛC'wæ?ít—¸9ˆ[?—·éæ<Í?¤3'‹ä3r?HÜ#‡¼?¤ƒ\ðƒFÚ?Œ
šðþT`4FGL J1258.6-1759¿ê4ÜÅW@FkÇÞP'ÏÀ97-Xþž×À;êU'þ@'°«@ݝ«w?°n²ÿàå!?Á–€JGÖ@I¬¤j®@[Ñsz¡?ã·íu?¿Ý`¥\E{4¿åµÔ}›6R¿äýÄy¿êéý)‹ê"¿ïÿùStAGNfsrq3FGL J1258.6-1800PKS B1256-177?õM¯?†"ãwN?p·}ÔþÝ?láó›Y¢÷?"Àû¼Âõ?îé±b?ï}_CÛö?Š"[Ֆóí?RÎtG?déj'<ª-?ŽN`ˆ\¹¼?ˆOwԅˆ?î\¶šH3?"5"3éÓÔ?‹ô,˲«"?'Z>ð€$S?£7"CnÑÎ?Žu¤—{ù-?ï©ð¦ ?m­ƒôÒk¥?`Ì«· ?PÏQ.»?†¾R(¯þ?jа¹]T4FGL J1258.7-0452?¬‰›öpS2@LúRv‰ÊÀ:Úž´æÀ<_ãåî@!wãۇ$Í?ú—FBÐ?ÊRøur?Ìçø··;ì@Îå«Àä@‰þЪþ¿ãtyŸ(NÔ¿ïÿÉy[5±?ïÿç¬L#Å¿Öèq²Ë¿ÜŽòâ
K³¿Ý»u›AGNbllRBS 1194?î']HîÕ×?£×®y?]•p:3Í?]Ò½mDS'?¥íï>˜ð?£—†ÍYÿ?îë|@UG??§ò*­˜k?dES@Ú®Í?tØ1Þ0ˆÂ? æƝá1?§Çæ0É?ìLÊr;¤?¢e"òSî?x·jEÞ?in_)¦¼Ì?ºjÕÉÅ?¡ç<>ÓlB?ì^¶r*1?¢&"<4'?n2Kú$_?k"Òˆš ?¼]ÂÝX?¡ôW†ƒF4FGL J1258.7+5143?åÄríw+@PWÀÁü2À; ¼£‰ÝdÀ<¥~`X/l@1ˆ°h=+@懖ü?¼žWµs•¿·QԞ}Y?üÚÕٻș@ÚÉWLm?í}î¸u'¿ë¬dAÈø,¿è†çn2
¿Üë›D«¿ë/˜Ÿá²?ݘœä§´åAGNbcu3FGL J1258.7+5137NVSS J125825+514225?îá Îr?¤(üÅ¡Ì?ŽéÍ?ƒƒw¶Ä¡?§Éw‰¿Ñè?¡¬ýÍÄÆÿ?î›ÑRAœÐ?¤¥¸èömX?s¶Á°œSü?€Ž;¬e|Û?£Ì¥Ò¨Š?¢:À:zé/?íd6ñH»á?˜÷†]hĤ?†³o†‹I?x»ƒÍhÙ%?²ڄ÷oŽ?•ýbül¬Q?í®35C¼&?š^íGݤ?'ÁÃ7:
?…²Rmö+?«»ë(( ƒ?–¬Y4FGL J1258.8-2219¿ì³¬åH;%@DA¸d"À8ŒR7Û9À;‡Üßi‡ƒ@ÏZ/Kr@¦áÞ¬É!?¤h_ž¡?·î…?€¯¤@¶æS†Ò@ínοÁ!¿Ìl•?ì+¿â8ϟý¹¿åg­Ó
¿æZ§K39¿èꀥ+ô¿ëʶDËAGNfsrq3FGL J1258.7-2219PKS 1256-220?ïM¾,ÚÛµ?‹r·=™?bʹ`Ú?X;Œ±®Ã†?"á"]?ŠºÖSõw0?ïŠyÜ&"?ŠMÉpéý?Ióëì$?Y¬ÇèõYí?‹ÂJ7™èÔ?‰7½[os?ï$è#8Qå?ˆTÍa(Ô1?v°pzݕ?rg\#:?•¶÷|×ã?"Í‹+"Ý4?ï½Þt>ƒÊ?k´JSç˜%?Lìëé?@ë?Ÿ7ºb?}s(}ÌÞ?i×UŽM½æ4FGL J1259.1-2311¿ì<-)ȧ@Cґ!%¶À9'u°ÐîÀ<
ìíԄQ@Ab…Ü#@Tò»sÞõ?¶‹4|?¥0â嬱?ëÝ[IŽ¿@O×X›Í¿ã‰è‹o4¿Ù£¤ÛA¿ã]'âïj¿ÚZ›WûQ¿å<á1ޟ¿Ø'·þ¯AGNbll3FGL J1259.0-2310PKS B1256-229?ïå³úGu?ÔUu3+?4›l[ø'?UÑz&ìÙ?heÞz9z6?Žñcd}²ã?ï±6pZX?…Ü5b=$?<̱0Š¨Ó?Q@iÍ·ˆG?'ÌeÎ?"a¥3跇?ï3rèp?€hnu?gþ(ýc"~?`«'gOR?–ŸÚQöŒ?}÷GÝÂ?†¶?pz#žcÁj?QXž=2‡?;–[Üü?†m">°'Œ?oé)µ—/Â4FGL J1259.5+2332¿êGª}[d@U~ªâ—9mÀ:ÎdÒ°,À<D(v@Îý@¯Ígý?@ÍDƒ½?ÄBðëe¿³t¬¾ÿœ?íä¦Þ%»?ÿ.¾+Ê3?¿â‰€Ç»–¿æØ^NêÊ¿èïæb.ï¿æûƒ¶¿éO}¶åû¿ïÿò~#¿AGNbcuNVSS J125936+233047?îàórÎ8?³4/ÍÚ
,?"šÓ#'bb?Dµ®ä-?™"(wΎ?±âö•oøY?î'W­°¡‡?§ÒaN®Rx?1=gü¦?ÆÆè&%^?£Ž5ěè_?£oû^š½w?í)+S¢Hw?˜­hØ©²?¿È±Ì]?Û2ý%tg?²¶upÁI.?•+*c‰ª?ìç"$àgq? Ô›Éÿy?Ÿ-	ÓºÓá?'ú×JÆx?°ø$d{?™#ÿÀë4FGL J1259.7-3223¿ïû;có@>r螺jÊÀ9{f¶~¢À;ðítA@èU³:Õi@–ªú-´?²=å~I‡?Àf0 .H¾@
Ä.béÚ$@µ¬]@¢Ý?ïû)ƒ£8¿Û—\¨wƒ¿æW!U;œ¿ä]sYN¿ét7	‰¿ïùûn Ç‹AGNbll3FGL J1259.5-3231LEDA 4075145?ïÔaÍ]2j?r泺Qm?Yّïšü??mi­*"´?n±i«›?f5:œªj?ï›ç,#•?†WoÚ´?L§ÜQ֙Ï?Z…-R9Õ?‡;·1ýP@?"¡lûÆ?;Ên?Ž¶'؝˜?ƒ·"ʧɵ?x–Ä©s¡<? )µæµ?‡i?Lgo?ï\,ÃKÑ?y	Íþãâ—?m´6ë¤×È?['Êڝ?ÃàÁêº?v ³V	øþ4FGL J1259.8-3749¿ïûµâ
Ý»@9²c"úÎÀ9©N¬5}À<4\¬©@×@û6½\@΀ÌC:?²­¢ bl?sLù7üW?¿3ƒåþ!.@2Xª'
¯?ïé»ðÜvŽ¿àËXߕ&¿àߪõâoÌ¿á‹}w$$¿â፞¹"¿à®þúGAGNbll3FGL J1259.8-3749NVSS J125949-374856?ïŸIύ"?‰W»7"ñÁ?Qèl«N?Vˆ'¹ h?†
½¾‡6ý?‡I‡ƒòç½?ïŸÕíÒ"	?ˆ¯D·+&?GÝ¿]ÑJ?WNmÁ@Õ?†Œ¨•šm}?‡OY0[Æp?îÓg%6€ñ?ŒÈ	ˆýp?kˆÑMû?` ½3Y~Ž?¡
Ÿƒ g?‹"S{w'[?îìé¥ex?ƒ÷Õ±Š?z"é™?aº3z‹C?›Û*OŠ®?€¢vá:Ãÿ4FGL J1300.0+1753?ȗaTò@T#ôörÀ:¶K̇,°À<|÷¤ëá@
º´2w@pÂàºÀ?ÃÆæþ¸?Ÿlp&궩?Ônw⏬±@›îÀèh	¿ì'+ˆDÀ?¢›+Ñ¿çØs>f6¿çE)Õ¼_—¿ïÊù=n˜?íýgŸKŠBAGNbllSDSS J130008.52+175538.0?îëÎvÎíA?™}jՑ?}~¢+›?x:fL–AÄ?›DÑ}—q!?–™ÁÌ1L¤?ïCK	‡?˜»w€?a@2Z&?nÖc$ir?•n›×#Ël?•à[âÕôÝ?ìŸ~Q _8?œéÚ­é?˜Ójþ@~?‡Èٞ¢Ø
?µ؜=v?—åðºÝb?ïÎÖó'?"Á
…ì¸3?…NӉÓa<?v¦$+¯±?'¾»\£ÿ"?}Mu8ß4FGL J1300.4+1416?ºLy•Ã Q@S>iƒQYÀ9tùòŸÅ-À<<Šk(m@_öèª"ÿ@†dÆS6?±—"–}/?µÝ';¦t?ûÌO~ÃT~@j«²¿ËÜNõÜeœ¿æ£¬!Üs´¿êHõ!¬‰¿åòI(gþ¿èò%ìù'þ¿ïü±®¤AGNfsrq3FGL J1300.2+1416OW 197?ïÝn1°Ñ½?k³Ø=p%?XM Ëf¬y?Q3¯'n?fjýézìp?hލò_õñ?ï[TxËZ?"=è'T¥"?bþ—øvhß?vñÛ÷£†ù?'<'q×Ǒ?'\r§ ¬?ï4NFÀ»µ?FŽfêš?p£º+^mÛ?gƒ`§o?•MHíÞ?zÿY¸š?ïX‰t?€úbá…:¡?‹¯u^È-r?|­JíÆ͔?|\‹ˆ'™Û?g»$RHA4FGL J1301.5+4413¿ëx;DÆûÊ@R1×Ûô‡ýÀ;Q3Ï:eÀ<×ÊZ+Ł@4ºuÝ&â@i[»èxû?™ڇ™x¿ˆ»Ö
ù3?ǵ­áÐ*@/xº{çW¿ë‹hH¾µ³?濞`¨·D¿ç£õ¾¸¿×|ÅW7Ÿ¿èŸÐ_©]Ý¿Å[¿XðÜ÷AGNbllGB6 J1301+4416?ïÆû±á-?vš~ã Á"?P"S"U"ö?H•Ö³ætÄ?xõíAúü?ujRB¢ã@?ï·^ÞÚz?'öAoâü?8ÄB:Ç?Ióìf>†?b&9Y'F?'P_ô8–?îég¨º4ç?…à
¾•?mæÓ^*…?dKßt5L}?ŸHM©?"YPáî¶d?ï»q=f	j?dþ‹0n¸´?b"s©Û…?PW0«Ò<Õ?xý'ʦ]æ?b;lÏó:4FGL J1301.6+4056¿Òq¤¡+@Siì,äeÀ;*@tdVÀ<Ö=Jä*@ &H½´"?ý
‡¶B?Èr_™ãA?½N䔔¢?õ")'°I	@µáL‹žÚ?¸f§>r×c?îŽCû"¿ÈydDùb¿áR"!7]9¿æ½+o"O?±Ô¼ZcαAGNbllRX J1301.7+4056?ïEA¤
&?"I17¦£?Pû¦
¿lÍ?Gè›´Ì3?:ÕEˆê?ƒ®‰1¼?ïvxáÇS?ýã5Ÿ*?O«í°Ò¬*?_±®DÇ¡?‰ç¢ì€ÿý?‹ŠÄhp?îqËÖ±c?ŽÓæÒ/RQ?o¹ú­Î	F?bƒ,Kž?¦óӗ¸	@?Œ²«ï%†?ï=#j‰£?
Õˆ˜u?~qÝ̓@0?k›E"Ø'N?•ÛäMû…?}…
›iª'4FGL J1301.6+3336¿ÝœÏ¢Ó~@TÉØ­«ŸVÀ:z/w¼ÐÀ<t[íf H@êÑ;F}@cH9Tµd?ÏAQ'Ó?®…-âønw?æ}+Ç.'@ä-̖ñô¿çºÂ^3çä¿ã1¹€¿®¿æšýqÛ:¿èO–áXu¿ïûãp}@¿ï´ÉÀþ¸WAGNfsrq3FGL J1301.5+3333MG2 J130126+3337?ïàf€ˆfƒ?p_'Çø•?E_KSÔ?C°w²îg?jA¬´èµ?lðDêä¢ð?ï›Ö¶0RV?‡&ß¡Ð?H·4Ý{Ä?\í$œö?‡~ß&®¼?…®b%?îðw8ÛHM?‰LÙvÍc?p«/`Ë?^iÞP /?ÆT_?‡õ÷QÓýl?ïUi:)Ó&?zj®sy@?|F'#Šã<?i ¤»²MP?Œ'pcÅÅa?uìk"ÉãÌ4FGL J1302.3+6901¿ßÌG€G8@H:}ªOÊÀ:ëè&Åf§À<ʞc,ö@bdþ²M@›?{@?ÅM%ã‹"?¡ðþ…V—?ÔhöÎþÖ4@UÞÂî| ?î²k!·	í¿çM³9ä'¿è-ê¿îI
{^¿ÊϵŠeõ¿ïþ2Àœ'ÈAGNbcuTXS 1300+693?ïí©a˜·?d¨«¿²î?R÷Ùb{?Z§šìýÆ'?Rù§c½1L?Y΋줺?ï8¶L/¶?™Bº
¶f?[MÓ=éþ?nOÚI
¸?—9x	F*€?–ël7´fR?íéÓÙkãì?"[–Á?B?€Æâ['Ý?rÕÊe‹&?­;P°ªÜ?ºKå`^?ï¼k‡´?k¶>#DÞ?bœ,·Áë?_Þ¿^tB«?x±3à–œf?e(œë˜4FGL J1302.7+4750¿Ë™]‹Ãºw@QJS5À:ûâTôNÀ<¿cí@»õÊd@Xb—¤Í?Ä|`8Nû翶µ_©D?ðùV̕o@'âý:Ó»?¨gmޑª¿ìˊw½¦¿¿ç§{9\B ¿áÁCâWùf¿Û!²Ø/Ÿ¿ïÿÅbu@AGNbllTXS 1300+481?ïxÄ7øË?®B"'÷
|?zÚÉÄÿV?"LN
§â?"ŽN
M–?­èK¯yß?ïٓñ?œsŽfŒ0 ?d"ÈÝUd~?ql *…?š44rRµ-?šiR‰óE?íÈÛÏ᧜?½·.Ûý²?"=?Ys?v—5æ"'?®bÿr)€?Ž--@?ïWyÑUKG?"¿;O
»?y0SƒÀ)'?vÆÌn×X?‰aèͺ?~þp%4FGL J1302.8+5748?êîŽŠê ½@MŸ©\…<À:W8õêÓHÀ<¾r¡L%@ÐÎý'@Y?¼®q˜?´B®Ñ9C¿5¶p?I?åÃ"ÿßHÐ@sã*\J?bmˆo¿è=þ"Ci¿àöÝâžÆ)¿âEbk¯ü¿âe!«ÌL¿ïÿÒþÀùAGNbll3FGL J1302.6+5748TXS 1300+580?ïÁx+Ó\é?¢E°L?[²Èb	?'=zÙÏ,?xWi¤JsQ?›™æ"Á»A?ï¨Þ¿ôó?†.ÿhÑ'?BèÄWý'Æ?T_~rÒ?"™ÃÚðƒ?"ýÐX{s?ï
Róáb?ˆz†&®jž?p_Uì›ö?m%†#·?šÌWH¬É?†ñ#míÝ?ïÏFnÖ¼?_Ég8I¹'?bðl‡:lð?Pä›:ٜ?mÉ$¢	"3?X۵ƒ¶ë4FGL J1303.0+2434¿ëy¶\·«@U–Å—Ne¿À8Ì£Ho›À;ÃÀ…–­V@u¸"Ú¾@‡5ÜZßJ?¨ÎƒKŠ©?´Ýv=I¸@¦˜5‹'@ÎØÈ-¬?Óe±ÀVò«¿Ú¡Q¿tè¿â™ÀGƒL¿âUŽU™¿æ@&Ì£¥¿ëÐøÀñwQAGNbll3FGL J1303.0+2435MG2 J130304+2434?ï·á'Ɇ?z̼‰:â?Ft{¡ÅÛ?Aݒç­`™?€ ZEä@A?yȘv'?Hz¶y?‹B22[ R?MUQMŸ?_ðûéµÖ1?Š{ØÐð­?Š &C+?î÷lǦ?Šw@Ê©°p?{ed‰B?u\û‡¸?šL
²6j0?…0ñˆ*P¸?ïµ³ÖW?û?n.䬣Y?WÂX?Bs{?Išâ•?5~ďeŒ?lóe4ÜD4FGL J1303.6-4622¿ít£–6}@0s§ü2ëæÀ:±®£íÀ<AÓë¤ÿ(@¹èÁÊæ@¿@D"­Ç?¿—ç'ËÊ?Æ"ïĦ¯@ˆì9ò@fš%Ç:?ïôÁPlÕ?Ïv<È2^L¿ß—dqē¿åˆabñfà¿è×a {{¿äoØ ?¦AGNfsrq3FGL J1303.7-4619PMN J1303-4621?ïK!Û{Š?âÿuÿ?ƒ£ŒêïÌ?'1NýŒ?‰"ü6.m"?ƒ(΁˜·Ó?ï}Œí[ ,?Î{õnЯ?Yc¦áÄñ?mcMsmÈ?yx4[¼9?‰×†z°9?î4çð¼®u?"p0Š\?Œ¤·Þ½?'y'¶ïX?¥­WÆrá?ŒHl'Y¯?î¯YT>—?‡
ª-ș‡?'K՚YG
?n ¼žÔ? wuU€<?"kÊ/4FGL J1304.0-5539¿ïÿ%¾;˙@´Ì?ß À9ésÉ%x`À;‹)ƒ‡@äŒu™µ@1;â.^?¼a™¢þÈ¿§ïС²[¡?ç2t[òo@›yòŠKž¿¼Ÿa.Ä
¶¿ãk›ŸXJo¿ëÐOt…
¿ÝC =͕õ¿ïþ"þ?ïâ
;Qå¦AGNbcu3FGL J1304.3-5535PMN J1303-5540?êÿF·1Ó?¼JZÄ;ßh?ˆ¡ªÑ)í?‡u™Ý3?ÂxʂþÞ?»kDOjl·?è™þIá:Þ?Êo·hŒ¼—?†ôg¥ÑcÙ?¢›zá³½1?Ì(À^þI?ɂÒ?¸?å×\·"?°š –•?§·!‰7Æ?">§˜,?Ñ[¥˜?¬ò1Ąf?ë6c¸Ó?©'¨"ÁÓ%?'3XN6àÙ?rӝµáŸG?Â>[®¨?¨û·h'
ý4FGL J1304.0+3704¿ÖÉN1±@SíKƧïžÀ:ÚñfàêÀ<žÈ:£j@Á›÷—ј@;^ʐ²?ÆcÄÄ?±h^ÊKú?æ¢6Æeª@¹©ñb?ïûùá
÷¿à™Ò¤}"¿çڄßÄK¿á¦W¸M¹Ç¿ëKz‡…šß¿ïØODù"AGNbllWISE J130407.31+370908.1?ï
ìö¤Ý¨?—†+ù³—Z?e-¡tì?^µBFý2Í?›Ÿ›‹P‹?—¶Xeéú?ï½_P~?‹càŽ
?O1î©ÿ
?_ÎïâÄÖu?ŠI±ÆA@X?‰wubcµË?®7Ñ<?‹ÄwüG-?u¶ÊXi«a?h`:Ã	?£ÐkÑu¶Õ?‰^׏zÖ?ïtٗ¦?}ìè>ó.È?ƒŒì†9¯û?o1KRXëR?'k¡°3F?w¬~>8f4FGL J1304.2-2412?ÖÀ¼?®8@CH×ðí=†À9Ëúú݁PÀ<(ÒO̲@÷õÄè5?þNŕ æ•?¸òƱ¿S?°­Ù'è‹?÷OÙý6÷ä?ÿA‰BŽ?ë\|m8è¿Û¸¬Cë<O¿âkb^ÄÜh¿Ø6%€íü¿àk'³ò
t¿á¶}euüAGNbll3FGL J1304.2-2411PMN J1304-2412?–ó?"ÿ€ÊÅàù?wz•1wáG?j¸ÖnRA?¤¡™‡"¶?'Hh'9—?îd~;á
Í?¡BA‹"É?~5m[*êÅ?ƒŽ5âp¤M?¥ñn–‰ÅÙ?¹vN]?ìォÞÝJ?šDÍmC£?‹]çTŽG?x¿äƑõA?µU¶†ƒá?—?äOsµ?éOÃöE}?-€~H´|?­úYh,¼?"°–Ðüž?ÃcbYÌÞÝ?™•#Ûi4FGL J1304.3-4353¿éY¾/ٕ@2êœo6ðÀ8zËïW;PÀ;wg)ÚÄÝ@E3'¹XQ?ûÎU}àÖo?¥Ø‰n~7é?¸Lݾ·‹G@ÅO±@|÷xÇçá?ïéXÎG ¿àùoߌ¿Õf¸Ü*ï¿Ú
ƒ÷ÿ¿àƒákÀB{¿Ý_ò.+AGNbll3FGL J1304.3-43531RXS J130421.2-435308?ïåB<ji?lÝß>KY?9Î,-?;'7 Q'?gƒþô̜?jrã†à™ø?ï€Ct¥Ú…?‹@Š¤RP?U¿aóGÝ?feçºáE?76˜µy?‰ƒ²@`ā?îÈ}ôè>?'Á_õ)´?êÈT,Ú?"®El©ò?úÝ8ç‹"?Ž?u"¥«ö?íÿJÅ6|&?—-°çpŒb?nÜم58?[F]vÏ(?®)õÞÿêD?–÷(ӄ•4FGL J1304.6-0348?»žjÜ—#@MrK èBtÀ;g€t.¦À<¥Ó`dĦ@?d3?ýùÓ`dĦ?×@.C_PH?ß× ìt2?ýŽ0"óA¬@	/^Ä;¿é«æ¾š¨¿ìì©@։å?ýz¿ŽËµ¿æI;þ]éj¿äþø™q¥¿ïÿYFÃ2ðAGNfsrq3FGL J1304.8-0338PKS 1302-035?îûÅgw?žŸ½Ô›GÜ?j:d¢Pòt?h™ÄÄxµ®?X:ˈòÛ?:'ÄXá"?îuóߔzS?©—nP_¬?t5m
¥?ˆ÷GéL•?¦ÛS
¹?§pù­&?ì‡U‹ɓ?¡5›¦È^?"ÜJ1òŸ?'gÌ*Í+?¶Î3ԍ6µ?ŸØþÊÕÀ¦?îÏëÄk?•…—ƒ6@?fΩfÒ@S?Z..ªªLÈ?®aøj֕X?•)¦‰&©4FGL J1304.9-2107?ç™çÕR@Dл¡+^SÀ:bßÔçM'À<>-o|@š,œì	~@2ç-¡"û?Ä_DB™®?µÏžcWé ?ï'ø!dS½?õ¿Ý5¥©?î.Iq?栚tŠìX¿æ:)Çy§¿ã"9°ûµî¿à‡Ý~›<¿ïûï< AGNbcu3FGL J1304.9-2109PKS B1302-208?í0'y¶%?§Ã,_ëҟ?ˆk<€Y½Á?ˆk7hsª3?³n¢C .?¦JY‰ó¼?ìÃB¢*¶Ù?²Eµ;±ÁÔ?šo…5ù? ñîìÇ\?³J$Í]y?ª†1T¹É?ì`òû׏? /^W½±¤?"ëï$ˆø?"Hæfñ‡%?·ýlX!IF?›¿;y(s?å&ÐÁøÔ?®:íÇK9?ÂÿV^RaI?¬aª)éD™?ÆÀ^¥»f?£€à(]â4FGL J1305.3+5118¿Â5•iš^¢@PkM:'£À:îòüÀ<Å'o(­@1æ×æ@;Ù_'F—?Òü4g??Ý_+ÿ¸1Š?úY
wt¬@ò!°~ã`¿ïûUá³äž?ïcóÅ_¿ìoC"º"¿ê§Š$Ô¿á¤jB"ùG¿ïÿ³ÿÌS€AGNnlsy1IERS B1303+515?ï¸×µ‰üz?ªC`GU.?{|œ9?€9ÈÌÖq?`0=O¦?dþ<s?îJÞÌN÷?­-dà'¢°?Š";gù²?E%‹™=
?¤Êz´a.?¥Œç»,?ì¨-$\5¹?šØCJö²? H'Íï?žhÂс?²·¹
kI?"©J/ ½ ?îk´Â€ç"?"š&È=òí?Ÿ>dÔJCW?'±ƒ¢-J?"KۘÊX?€n»Ñá4FGL J1305.6+7853¿ì©Q§´Ü¸@CÿyÈCÀ:EFmCÐÀ<¯:ঞ@Œè0Uˆ@ðàpÀ?¸­G`ç¡d¿I]ÏÖüØW?¢Èè!ù
T@­˜¤§Ö?ï]=Þ1ùø¿â²ªפ—¿ä'›…,$K¿à;ú'½˜¿ç»üšð±®¿ãÑqw; ÀAGNbll3FGL J1305.5+7854S5 1304+79?øÂý?Á2RHS4?kö.Š±E?c=RRš{?" 6,ôx?}æwìZƒ?暴OR?"6?‰Ö/h?fƒ–˜WU©?s‰y;<†t?šÚ|c
Ò?'Ãq9Îï¼?íŽÊ2D¹?"ó½CÕÙ?ˆZ=ƒàx?vŽ2áU'?°~f½cË5?']qŠ˜Z?î¹êË·û?]è^õ‡Â?žSÇ˒+ ?ƒvÐ,ÿF?žôúÚöÕ
?…åM>¥),4FGL J1305.9+3858¿í=s,aK¹@Sq€ˆP›úÀ;"Á¯bX»À<ópˆÿ£@™¶¯T@·
è`Ý?ÍSÄ[d*?³G`ÖsY?å)¦¢@²"@ÖAj®u?ïúÀ~gå¿è™K`P¢°¿Ò¦…eZ!ß¿è17æ Zé¿ì;yÞhUª?âɛ?-±AGNbll2MASS J13053124+3855218?ë ‰&€Z\?½Fs¿F¿…?wæ‡ê{ŽÂ?'?h¹¼'?¾§&ªº?¼Ã;˟?'?î‹ìQRÒû?¨Î.¥~´1?qrguj??gý3x+?¥îä#?§­¤]kA?ìAõŒòW?¡%›èSó?•° ÝÁ?ˆtlXvË¡?¸"+`û¢?eI¡¤¢k?îKPGQæ?"ú@U`?'E¨Çä?r ‰$]?§WL'ÕÈ¡?'!°¤DšÓ4FGL J1306.3+1113¿Øc­xb@RmÛ"Ðå`À;1Óºý—À<£Êz5˜@ }¹!]¹?ÿÀëíúCþ?ÅџÅW¸y¿l‹.|'3o?¤ëÜ1™«@Jc]¿ïÿý±q&´?ïÿáÍì¿Ý ÎâP¿àÅ%ƺd¿ïïícEI¶?ïYà37AGNrdgTXS 1303+114?ï׋ØÀë?xwÌr?S`ºÝÿó?X	ðňH?nÃÉÐ?t;®jW?ïqRIX÷-?'Šj?-
M?TH×À?dó2»¬üc?ŒâGpéX?1¸IÈÐ?ì«Î¸ÓB?ž(Îë!èš?šj)H§&õ?T
ùqžg?´ÿìïœ2?˜ÎyöÝÑÍ?î0ވ'??"~ë*"-˜?Š~F…?¸è_µ-?¦Xp'6zÉ?'}çnëÕR4FGL J1306.7-2148?ï1¤"'.Ê@DuöM½ùÀ9ó~°à<À<,YÜë(@s{ϯ*P?ÿ³!Dô%×?ÂGFe•5?ÉL²`9ü{@¶n¡žJÙ@ ZÑ1áO?ïþá77¥¿çšf³"?ã¿Ðƒp!ûþ>¿á†UºF¸K¿éi¿·:"Q¿á^˂Iñ¼AGNrdg3FGL J1306.8-2146PKS 1304-215?íiüæüæ?©*'L[/°?£Cò¬¢Ï'? <ô}~N?¦Läíb(?žÐáx?í#É1¶?¬X=S°-?–©š՟¢?œ²xõà#?±<«/¼ç>?£ÝT0B&?êšû¸ÖV$?¨J` n?¬ ÛÉÈŠ?šò‡ç?½´TiF? ¬³Ò9¡?é
cƒô?¡kXBpR'?²mjRí†A?"~
­B0ö?"ÕHyl?š8³l€Â4FGL J1307.6-4259¿Ìºð÷ys´@3ÇÅ£ãŸÀ8¦17°pvÀ;¼-Qqâ›@Y24…˜±?þvbBw†?¤­r¿e00?žN%ûÎ?ö˜l¨ŸÆÚ@	É~8À¿ØàᬭȿÍc)Å÷¿Þ$_۲ĿܯD3‹ž¿àÛçQ³Pû¿ÔcÛÝrAGNbll3FGL J1307.6-43001RXS J130737.8-425940?ï½n¡MÃ?t¬¶ôÌ3¶?DªŒZÐ.6??=ãü‹_ä?~³]Î"k?tI†aÇ£?ïcŸÈjë?'Fò/6´[?\Ý@kr?o³¥6¶k ?'Ã25>›Ù?¥Ça˜–?Ú;<
?"Ü|ç'9?rö–ý'K?ozs{ëRÖ?¢ç|¨Zv?'u¼D ÓÅ?î"CX°ê?'äKžx'r?†ÒµœÙÈ<?rÌBð'¿ð?¨'žP?ïC¡i#4FGL J1308.4-6706¿ï©LÎÿpÓÀ*"'AÀ9!'ˆŸÀ;™)†âñ@ J5Ù*Ô@½¾hê?´uÞÝp‰?¹YÝìÚ´A@ÿ}>@C@ké?Ÿ'?îçuû.ßç¿ÓЕ"60¿ä¬j¹¦¿æ:"`R%<¿äXÞ=¿ïÿÿ" 5•AGNbcu3FGL J1308.1-6707PKS 1304-668?ïªtµ"V?~qx"ô?7'Lûô=?2Ĩ;íŒÈ?"Âr'
û?}Ùt«í8?ì3ú‡)g7?º—MÞõ…?DZ+5
¦"?bñ–l…î~?¾7wpJªø?ºR¾G,?ì
Á":? Ûr;â­?Ž÷u#*©?§î+ê7?¸3ø£OxÚ?â©Ҟ-?ãUP?‰;~€©e?mŽòJÍ`?Z!4_GÑ?£;/­(¾!?ˆk€£n›—4FGL J1308.5+3547?è©+'ԍê@T&»ó¡MÀ9ëÂÐʈOÀ<f½Ž©|@j°†5á@tÌ?ß ?µóÁI5ÿ?Í[‰ûkò@¯ÿCAž@Z3k	?ïnÙgÒ¿ÚÊZ+ŀ¨¿ã¼œ2Ñ
¤¿çGÏ[¦¿ëä¡ÿ¿ïÑ ;tJAGNfsrq3FGL J1308.7+35455C 12.291?ìóܜn?²OÛiã¹?¬®"ù{;?¥ý=F?¤ ô	½ß?¦°k™¼?ïZcÖ¿º?"}¶ÿˆ}?gÇE+'}?|ªŒ­2q?'ÝZœ'£©?'þÏPBå?èx5vd?°Ÿ¬ý/?ÁQ1VGÂ/?¨ž¬fÿ?¸ñÛ§½[.?£%ˆ|gw?ïN4Àƒ«?€KÜÉà2Q?‡wƒ›sy?wš+†óú?"ÕXtƒ¡§?qö.Š]Ý4FGL J1309.4+4305¿Ôù!†"áH@RhVWûi˜À8êé—îâÀ;ʟGX"&@ðÀΑÈë?üMJ†6‡?§xæàcr?µb»¶úÓp@_$•á~5@aÁŸÈê?ïêv–_Rv¿ØHŒ¡8ŸY¿×4B<e‹ö¿Û}»ÂŽZv¿âÖùvy!¿âçrj€§ZAGNbll3FGL J1309.3+4304B3 1307+433?ïÀÍô×?u­"ÝÞh?Qèö6,Âb?L,üŠBU?{Èo¥ã›?sƒ Ç"§Á?îÚø«€'?¡=è)¼CÚ?vBg<?"¨´KoR?Ÿ+ù¶á?Qì@Ü«?îóÙVº‰Ò?sý¢p"?Ý#;ù\"?28ý³®?˜–CŠ²¯?"E÷¤œ¨í?쏷"=Q8?žÔi'³ê?™!¨t%Ó?"XÈAÿNt?µ9ÙÁ2?Ÿ?›áÇ4FGL J1309.6+3718¿îwÅ~@SÇiÂ;ySÀ;¿B$g¾UÀ<õ²6ci@!Cš
,Õ?ýåù×ÇÓ?ÅxÀƄ3V¿¨ŽïÇx¥?äòÂàdÚ?üê#!BE?ð?àØ ÀaŠ¿ÃSGOÊÄ¿çñ-Õ%`ã¿á…\–$?Ä?ՂþÍ{AGNbcuFIRST J130948.8+371651?îíï¤H	þ?¦=ºÄ÷	?Q'w£•AH?VoüEÿ@"? —Éþb¶
?¥â/ðbÑh?îQ"a
rB?¨ß—sœp|?z–žº[|?‰š®FR›?§"æ+ѐi?¦zê'Pݓ?í7EÃÄt?šü>€Ï¤?'öYÍOs¦?uB¥j#)Æ?µz˜7íè?š9EÏ?êzñS˓??°´L/ ×X?ŸÉüå'Ô]?™•àù›É?Âûxw?°Œ¼›34FGL J1309.7+1153?ä­ýJ²Å~@R‹">iƒÀ9ÉQì[ÞMÀ<J@~uPå@-Øjå§@%ð|Õ=µ?µ ÏXmTl?¯S"'Û9?÷–…³2ÇÓ?ÿÄ¢–?è*·c®ü¿¬À=àÇg¿ãshãh­¿á'­Ãó	¿ç¥¹Þ²§¿ên¹PïÝAGNbll3FGL J1309.5+11544C +12.46?í£Š&xÙ®?¦áü²8?ƒ©6µT•?v:QБƒD?°nˆ'‡û?¥"ÆfÎT?íÚû*ªM"?±ßl:óVÐ?'b›UZ? h't>ý?©°^"?ªM8Õ"C?ì'˜ÀëÒg? ÄÌ¡¶3§?™

$º[?‡á
‰Ç?¸ö¯rÕð?›ŽyˆþII?èüÄ-íU?ª_‡£v#Â?Ä£¦ŸAõX?©yû¢?²0Ì ª°?ó~14§4FGL J1310.2-1158¿æ/š½¹'@IPØ]ú‡À:KÏknÀ<UBí»YÞ@ˆ_X@$(ƒ¬ÈK?¶þ"n\T?'¦Ø؄ø?Ýô^´kW?þ&'Ë¢¿ï(,ÚSž
?åzVs'¿âœ°ožôL¿ãdT"—½¿Þ¤‰ôaf¿Ó°
ĎºÃAGNbll3FGL J1310.2-1159TXS 1307-117?îí¤$k4?"hØ¥þµ¦?ph LX*«?d¸$@îm%?ž1s_vN®?'
1NÇ?ï8N6»?šJQm-x}?bß2%ñÝÄ?ow¢GB¿/?™ý1zìä?˜)Ø÷¦5?í] sùu?šÉÆÜ<È®?o­?W'örDy?³œÐXn?–7S7ô7?íj´'¸Eo?'ÁdOmWÁ?—èãy?íۜN…n?­`µò³l?"È?ˆ;4FGL J1310.5+3221¿äô  ã@TÕ=1¹¶pÀ8M_ŠªŽÀ;[ß-ø`Ï@³±_^	v@eÊål?¤6NàQ¨®?«DTÚ<L@`ù£v'@LVjoàc?ï%tc+Y¿ãE& RÆK¿äe·]®1¿äF'ÌÍ£Œ¿ç™!ú{²¿éécÜHkAGNfsrq3FGL J1310.6+3222OP 313?ïÚöŒ]˜M?hò9cf®Ã?Uçˆ×

?QA±ï—Ñ?j¯Ÿü,d?elö)ü¾?ïyiF¹Ø·?'}ˆò9¤?[@\Õm¦m?q¿†Nw›ê?Ž=¢¶Üo?µ¯­þÕC?í³:S¡6?œç_ª{Ôy?ˆÔ˜&±n?'±‹þBQ?®—8‡ü@Q?™V Îœ?îwf—"?—Pü‰›Û¤?Œnë5¸?7È¿´¹?¡"6zÓc?"zMÉØ
}4FGL J1310.6+2449?î3)ß]¯@UG"…]¢sÀ:Œ—f¹rÀ<'Ã}˜²@ₓî‰á@o–Aö?»¯£½ú¿¥Ù«#ýÀ?ëᣦÙô@SqîYåO¿äêê>͛)¿Üº[_L¿ÛâCV–æ¿×¼Ù¥"cØ¿ì³+ ?:¨?Öôû?&£AGNbll3FGL J1310.6+2446CRATES J131038.52+244822.1?íó V ?³"¿¶å?ŽIӍޑ?"ù|"5€À?©)í%²®a?®àëËtLp?ï)h,e?šdR¹?hõõŠ{äI?€X׶s=¨?—´;»á'?—g´•j)?ì+9#CHŒ?¡¢åÎÇ ?¢qÚ"¬¬?"ƺrO?µmI֛å=?›HI{™ü?í¯µ|+/Ü?—òW×g?ˆ2uî£g?ê·d}é?¦@U°ž?…¯Ðp4FGL J1310.7-5553¿ã_í¨†é¶@ˆ.¢ªºSÀ9§¢KïÃÀ;m$²>¬@B;䲝@SsD›:"?ÑqÉ—ïu?Ør­™+@Q˜ÿ?æ @o¦èa¨¼¿àïG€È|¿é'5deÛ&¿å)™—Ž¿ëüXáB¥—¿î¢‰,d?":#«š'AGNbcuPMN J1310-5552?âÍÔÁQk?Èïá+£`<?n'/¢"?j‹… J?Ú('Zþ'?Èì¨^Ö(ä?í¢׍?½ë¹±?yJA5<\?–>xÜ?µ¦KïÒq?¼V:J 7?ãØ÷@<$?±J؛ŒI?²ÓRšJ`?—çï¦?әQ+$õ?®×ótß±'?íÂS2\óÙ?œqzh«`'?XöRȤÅ_?GÿŠ«°[?±‰!õÎ%?œ@ÔÂ	4FGL J1310.9+5514¿åGÞ&¢'M@NÔ
9À:[FóÚWÐÀ<´Näi¡"@˜GŠ®X@ÅP^½$¹?¸ÒK¼ÁçÁ?§gƒò¾N?êwAë\ÚÌ@ý;Qå¥â¿´XÿJ£gN¿åÓLãÞaJ¿åœ³"íbo¿åöØ9¦ë¿é¥ÖÏÛ¿ïýO¶÷xrAGNfsrq3FGL J1310.7+5515TXS 1308+554?ïP"2ê´/?\Ùk"?x
{ÃÜ?mqYæ{ö?ól‡q}?‰|<sQõ?ïcÅ]î?éÁÎ}dÅ?XU¹òý·?hõÝF?''C
,?ŽrùÊcÞY?î¾Vó]?‹1¤ìÿë?vÿm›?qԅ⫌?¡@#+˜º?‡iVµº?ïKówà+?zc¶Å6¨?‡E
Ê+3?q¶ž7\U ?…¾=ÏB?p<zLú4FGL J1311.0+0034?í'WüdÁ@OƒqC9:´À:&­~Rì6À<Ìóc9‹@ Þ.Iš@þM œÃ?·ó;K…w¿¢!¹€Yé?éß[zz¢@7Œnbß¿âEU	FП¿×Oê£øBF¿ã{E†S¿àîÿA"¿ÜÓÄãŸL¿ÙT—¼Ÿ®AGNbll3FGL J1311.0+0036RX J1311.1+0035?ï±þɞW?²³8Ö¾?qü5݃÷7?hOML'¨u?—겯k7g?–6AqA?ïk"EÆf?Ù'`$¿°?Rèa^Ø?`vÑüÁŽ?'_–í)D?!‰Ÿ?í-eõž8?šk˜6î?ˆàÙPˆr«?x$¸8Ùª×?³xµ-	ÿä?–'Ñ÷=ªp?íþÓÝ£?•®½íÖoP?Šk2t¾ÿc?xÃîðfCn?´*£{4?•Äê4FGL J1311.0+3233¿ÔÂúªÅTÍ@TÆå6P&À9Ú J"cÀ;{Ø=CWn@®´2ø@.‡$L£?ÁÍÊùõ÷?ÐÖ\˜‡K@3Š™K–@IVå¿âÙ¿ë–ñÿ6V~¿¶ªåò7Àa¿ã,iöZe¿ã9ŠÀÏ6¿écÞAp ¿èØJCðð™AGNfsrqRX J131058.8+323335?î?>•—S@?®¨¹K
mª?'®¤œ˜Yý?"ç¯3z"n?¢´ÄX>žî?¦T¸:l?ïjPÑÙÎU?"p,â$ù"?_âKUQ?ql°¬S?·Åƒá€?þ*55U"?矏–!¼?°Œ]T¿>‡?¯¿Æ­ØÏ?›™2¶‰š£?ɑÏÞ1tŸ?©Ø6]+šl?êc†°Öø?ªáµ<=?Á4›K?€é™ûœ«?Ā¹)^p?©Ž8lG£4FGL J1311.8+3954?ã>c|@@S"Ú<÷À;‹ì §ªÔÀ<ñ令ß@ œÜl'¡?þɋϬ{?οUÀÑÁÔ?«fÝћ¿?àóîå%‰'?ýùö{œÙ?ïý'w>$ÿ?À7`"j[¿è™â"µ.K¿Õ4¸#G'Ë¿Ö<‹Á¿¨w¿äðÖÍÏ3AGNbllFIRST J131146.0+395317?î¿Ú1çM?¥f¥J ›?T£¾*ՙ?QA^y9E%?£]>ôÊÞa?¤øú°ÅÎO?ï5"ník?šE¬Ír×}?`s¨ëD¡?ǼÎZV?—?9½ê?—¢R6S?í`¿¥o?–'0&Յ ?vóŽªÙ=­?dxÂDÐN?²Á&ð.?•>`N¤ƒö?íûjaøHÔ?"ð—†WŽ?‰ÉþA?~vVó¥°?©×Ú
ƒN?'ô>aÞ¤4FGL J1311.8+2057¿Í?Ò9.†@T'(ÂzÀ:³ŒbÀ<k]Îpk@±ObhÕ×@
aûc?Åù‡€gny¿Àkí"ì±?ú
Â*²[1@"Àl—¿¼ Ì"Áé¿í66Œs¿ì£ÙŽ|/&?ºÕÊÍC?¿ïÿöùŠp?ì:G#ªÿóAGNbcuMG2 J131144+2052?ï"#M"Œ?›}‹]Gł?‡Ÿ¾#.ß?šÂ5¿Àc ?m€¡¹ß¹?v©¢¿Q>ó?«±»²?´.ù\ñ?‹(@ŠíÒ?ª˜^૚m?ž™
DQ ž?¤ôôå¬iÊ?ìáÃàöÑ	?˜àµ'¾?ŒÌ3ùDÐQ?€ìõ?µXZy Ý®?–Ìì˜QÐh?ï‡m'›w?Z•VJï?ƒM'"IX?/PíÞ>?u®ª.²À?tv‡§Kô	4FGL J1312.4-2156?¶‹=á7@DUóFí$À8µÁÉc‹ÁÀ;¥'õÉE@ýêAÞG?ý:61ë5?¨ŸCãÀÀ`?Ãc>Ò£¦@Ò­`ûH@¥ŠFjr¿áËOK¿ÍÐ-hî׿۠¾øN¿Ý^{ ۑ¿å«(m"˜¿êIÈ ÈdAGNbll3FGL J1312.5-2155PKS 1309-216?ïÛj""l?hÿá­=?V×O¿—£?UÞís¾¶i?i'ñÄÉÛ?b:ù¾"×?ï!Š.Ò??—ðãpnÕÆ?eØùqí†?r"XOʆU?™·æ‰ÐY?–"•œ…?íþk¥Å.?œÜ<|Aæ?ž±¬y?•·j3Ô¸?¡ìÔ×h?'˜ôPM¬?îûòFEª‹?ˆ_tØ5?nub½}¤æ?[؋´fl?œ³
ߚú?†îéoõß4FGL J1312.6-1900¿ÙSQ¤7'@EÈÿ%¿­À:ê ú¶ëÀ<|K2-y¶@ …½ôAÛÃ?ÿ}"jŽ?©Â܉s?"†_ޕ·?ÅõÛĈ?ÿBX•~Í¿ë‡e_L—?ïóÜÁ6–•¿ÚÙ]ÔÇm¿áőڈw2¿ä†'ø»h?º)WgEžAGNbcuNVSS J131234-185902?ï©4áÂÓ·?{ô-È¿[Å?R;¯˜û£?H¹
r¦Ö
?ƒkQœ+ô?z~ÿ¨D`ã?ï= âþºŸ?'AhÉ/{?V9Þ.ßë?a£tÛ%?–èE½:ºi?K41  þ?î#PEtè‰?¥ájÊ=?xþ'±¡:?f\º»p±?ª«8#»CF?‹=(ƒÉ´Š?íIi'é°m?'Î"—äâE?Šœgº6Ë?vçJ4B6?²a&yr5É?'ë¤"XÒ4FGL J1312.6+4828?ÝÙ@QÔªà"À8‹p*ÖmÀ;ÊPSÕj*@²6¡&Ö®@‡¤WÙÜ?¡HÔ|ì™?¯¾"¤9I@>vû	@ R3€5¿µùN`
VÆ¿ÜÆày§â¿ã%p'Iü¿áW^‹¦'¿æàTÔmªþ¿ß—ô}ë¾*AGNbcu3FGL J1312.7+4828GB 1310+487?ïíÅiµW?X6<Efò ?2µÐ
?+$I0ώ?_ò+¡TÞH?WÛ_>õ?ï­ëJU?"­xº—Ùk?FŽÌ}û'?Yãý"¤Ùj?ƒ@¢ÜÊC?ƒBQÝsi@?ï%øšµ?…AeŽ§à?tTC !y?o5âìè=?—(jxæ`Ð?'ÝAyÊÁ?ïÿ¬<~ ?åzûߔ>ÛÜáÄýè>×¾X½I?¸RƒL?W'óZÕR4FGL J1312.8-2350?Χ(xo'€@Caÿ.Hè§À9»¤ûÍkXÀ<*b{ö@ 7™Ig¨?ûîPrß?¸ž·¥+?·í§¸Á''@eÂÒxy@Poĉy?í¾aÔU¿àR*ڟg¿Í'&]·Á¿ÞÅå"S·¿Ò‰ÎÒ`‹¿âÍ
>××AGNbll3FGL J1312.7-2349NVSS J131248-235046?íý5 ¸?žÀi	ò©?!‡ÝÌL£?°3ËÚSy?«äDqkV?™6'	[?îç/@?šÇøTv?q1ÚíLú4?{¤
çc›,?žÍ¡@Ù±?–¶]ä˜X?ìªl³Ìi?œ–
2'u8?‹EG.Páñ?|{î§s5M?·Cñ{қ?™}sìßÙl?éøØÉJC? y
ÿ<?˜Aᛍ ô?'ZÑx®ƒ?ÅcÁi2Ò?ž'ÓsÙ×14FGL J1312.8-0425?ÜúÉÐ0Î@MÜð0$À8åö1J%À;߬ÂkJ@ŽØ™´œ@¤u_þmY?¬wìÃÂ¥?Å'Øa*'P@[oŸË@hJã©K?臕ÀÇ
¿ÛAGÞeü^¿å¨ïbxñ¿ç¸Ž·«¿ç'£²ø¿ïÿK§ž?AGNfsrq3FGL J1312.8-0424PKS B1310-041?ïnÚI<Y?'jšø—?zíµ¢Œ?{µå§ÚÂü?‡B¢íVŸ?ŒNv²!=<?î·?Š-àïeW·?O´ýl2Ø?b
¤Üį}?‹äK푻[?ˆð€±:¢?î4µ$ùŒ?C0'‡Ü"?6îVñ?†a.Hc¨–?§¦òà?™û'7øÇ
?ïâÂ{©Æû?X÷'Œ—ö¥?HKÚ·Ã??±[8/Ñ?g*½‹"?UÁRX¬®•4FGL J1314.7+2348¿ÚXò‰c°B@Tò	ª£­À9;Ñ|^öÀ;åw¹u4@dçv¯Š?þV½+o"?®t*a"ð?¸ÉÏAq9~@HŸ¬R@€\óvè?ïf* ºà'¿ßhøÑî¿Ý¡¼þ£‰‡¿à˜B"пâúK '\9¿íÍ;5À¬AGNbll3FGL J1314.8+2349TXS 1312+240?D¾]Í?­¶¥
ø^f?L,QG6ÓG?Aå@FPB?†Ò©»õ™?­ºf߇cd?ïMvön?'"6[ìÍ?c`Óy°º?nŒítÒÂ?"äbœ;?ê{É`ø"?îím·÷?ˆ‡OQm¿ÿ?€{ИJ©ç?zz÷A¬ñ?š`´úi/?'B©ßì"Ó?í`MÔ'û™?•u9œ_ò$?"£Jc½ÑS?~D滄À?°¾ÅЮç?"ξ¥Eúþ4FGL J1315.0-4236?îcÝbFF5@4O~ÃT~À:&¤/õ'À</ßÅoá@"`3F~j?ùÿJH"®?Á5Yh§m?¥$Y%¶?çoPð³[â@̪7Ìu¿ïù>Ú[V?îÉCu –
¿æMà}ٟ™¿ÖëDÜþÉ¿ÇÃdCK"8¿ÖA_›ÆðjAGNbll3FGL J1314.7-4237MS 13121-4221?ï˜Çz0Õ'?‡yaŽ©a˜?^Wä$áÇ"?~Õx¥ ì?†$ï.}:?›àþî?ïj"i§¬É?'V‰ ?Y6Ü1•_E?gc8¦Ë?'ñÇ?í™©,?쥇þœ¾?‰àgÇ ?"ãπ'?w˜l@oÎR?¸7P/I*?›ÜË-%N"?ì"ýˆ¸ƒ?œN7ìÛÐ?…úR¾?y"5˜6î?¹ÉxgP¯?œÝ‹'¤Ùq4FGL J1315.1-5333?ÈÆ&JA—¥@"HϧÆÀ8¦m¢šÊÀ;RáNd"@Ù{Üpê@‡½#â]?«AÔ&?À^GG@֜¾H'@÷¶p"è…¿Ñ慛
¿à†Àyt¿åUD€ª³¿æ(°B¨q#¿éh‹¬"q¿ê_Sb'½^AGNbll3FGL J1315.1-5329PMN J1315-5334?í.՛.:ž?§VÆ[/[?k©O¡@	¾?ehe0ÌXn?µ¬©"*½?§5Í£\ f?ïy[]]ðÙ?›ð\¾FE?J#ÀÕEõ?bWè)ì?vSÃ:â?›?‹F¿/u?îK L	G?"L&HË?'nZäm§¡?v†%_+Ü?¦ªiB$°?'øéø7Îà?F҂ó?w3º
5h†?P)N0‰??AÉîFÿÓ?T©!™1ì?v Š]ªF(4FGL J1315.4+8453¿ï772W|O@@?·¥ôÀ:ØÙ.IÀ<jÑâ¶C@xIéW@"}€^_1?Æ:azÄAc¿ŸÜŠľ?׳Ûåž@–ŠýtŠk¿×V^?&¿ëpBRŠçO¿â©å‡ó¿çÁ½ªE
¿ïÕ@%Nn¿í€MÍé,AGNbcu6C B132240+850531?ïU؂(¡?Ž~Ü~R?qT#ëµ?m6£Âc?àì§Qðø?‹V¦ãÇ ë?ïAºn«R?—™¯&¿Z5?d­-*¼å?q/¨«ŠÎ?œ–³…>0?•l¤?»7
?íi'¼Oî0?–õýºf?ŽËã«T?;"|Ï?°áp­"?'±%VLÜ?îzdU$Ý1?‹£ôr—?€ö‹ü—®?pl䬲£?¤Y=
³?‰Û™wÖ:44FGL J1315.5+1135¿ëKê¼C_@R]­BÃÉïÀ:" Rñ?À<eïÎY"Ç@ îRî'?øú™ú©v?É#–=áã?ËÐá.ƒ¡
@7°pu³á@Ôüj?ï)³ʅu¿í¹´V´A¼?Ì´ÆÆ£gú¿¿›Gn©€í¿×{°&äp¿äÎK^˜AGNbll3FGL J1315.4+11301RXS J131531.9+113327?ì.R6æâš?²UX¿æÝ?yþ˜@ßkò?s—FB±}?¼í"ĺôi?±Þ¥pº+»?ï:–'Ó?È?™ï,Cîv?[F»­W´œ?f-J+ofõ?–øÏJ‹Å?—ºö•Î|?슿ݡÁè? W€ÜÊ»¿?8¢õ®¤¾?s.ÔVdĒ?¹'ì´<?Ÿ—º8˜?ëàÇU…í—?£¼·_û?€ºln,?q;Ú:i}Å?¾ùŽBÍÈ?£Áð¢4FGL J1315.9-0732?é"Ûƒ7Ç0@Ki"}ŠÀ:
뱔b"À<(^Ì>1"@ƒkµ/Í"?üO9#7=?¹…cÂD¯?Á·uø®@.d²1@@mdDM6ê¿Ü$´?b@'¿Ù²ÕÎÂE¿¨ˆÕü÷7¿ã!¡ŸØx¿Ýa'nê¿ãwקò"AGNbll3FGL J1315.7-0732NVSS J131552-073301?ïåj¡@ ?`Ș1Ì®Ò?Q¤"¼æ4?Vl¶qC#<?aÃLÆ?UAÄÚ"æ9?ï ózƒv¯?‡2d‡gt?B®tK³?RŽ7é"W'?†˜:pØû?†$N1ŒHŸ?îê¾à"z?‰ð.5̬ ?vy€ó?s
‰ßŠª?'…in#?†×E+U"o?ï}'¢¶L'?wi"\æÁ²?I}Õtÿ
?<×ô^iÓ?$?u¦x?w
ªhÂâ4FGL J1315.9-6349c¿ãì:¾l⬿ña၏·™À9ªl…dXoÀ:²/€ KÐ@'±…"@šTÅT2‡?Ò§9)í9T?ºM6iž2?äkž´‹g@T,Ž~]~¿ïüœž0Ø?îï7œ¿âöÙÑ.[¿â©‡¸Æ…‹¿éUDÀyWZ¿ïðdìé¢ÆAGNbcuPMN J1315-63540?ÎØ÷
ë"S?Àjím
½?¨>8mYÈ?ª@è΂/à?æ¿îY¾IO?Â,b{c:‹?ÆM‡š?ÂÚOgã?ˆÝåá\l?•å:¥•?êõ%X© ?ÂÅ~|G÷?ÊƅSâT?§ªr'n"9?¸µPÜ·š'?Ÿï.ÃÆ?æ7´p‹Ù?ªd¬ƒÊ^Â?Í.^-Ú8¼?®#CgÖ>?5¡RÝî7?~<­¯,B?è2»iò'_?®Z‹bÕǺ4FGL J1316.1-3338?ãY}M–®@<ôFs×ÜÀ8gõò`MÀ;ˆÏ×CHT@Ÿ­"Þ@GØåó?¡õ'	^Ú?²˜Pï0Ï×@c3á®Ü!@…Våb¿ÐÒ¸©)¿ÝÖ¾=<÷W¿å3¥´Z@¿å¼ä!}(J¿åUK Â€¿åZ‡5DAGNfsrq3FGL J1316.0-3338PKS 1313-333?ï©¢'3Øt?våDQmž?CL£-–À?:ÚWz-V?"b'Ø×	S?vždw4L?ï·ê¾.Î?€G~J~?A6Œ£P ö?P¼Ñ)HŒ?€ñç®?Já?~þdgES?ïÙªÛÇ'?‹XºœÈR?t'õ¿v¦°?m&Ìps?™@
4©qU?ˆspt?ïﮀÞ?PñèGF{v?&×zè"2?4ŸÖê&¸?^ÿ³¡3U¹?P`
€.þ_4FGL J1316.5+3013?㩏PÈøà@TëQÕQ×À;¬ˆô'À<ÿé]&KÄ@e°ŸÅ'¬?ûÒÂÊëK=?âÀžìå?қ‹vÁ'}?ö;¥wô-d?þ•ùqE'†¿ïý.)7?ïÄҗç貿ìV́¨Œ&?Ӑ¨"C3¿çZüۈQs¿ïÿ^Ô÷"AGNbcuRX J1316.9+3014?î×ÛH}zš?¬n‰F©T^?`gbfyß?c;ÅUC?¡{ÕQÀ¸ƒ?¬
Œ<ó?ï…ï­Úý?"ÛUdÍP?Wï(ëÀ­L?ouâth1?‹†/ Q+=?6§zy?ì¼¥°
{?¡4^«Àg:?Œ~5Ô@/?|›«ÜIFD?¶‹Åä$? >$ӁÏ?ïZ4þ°r?ˆ}ˆÞJ«?uƒŸ[|n¯?r[0[­#?Žºc•¬?Ühÿž4FGL J1317.1+6613?ë'ëòyQ@IYÝDUGÀ;D·éæ¹À<ÑÜKÅÑ0@ƒÁRñ©@|l—ØÏ:?ÂFµœ¬2¿§¨¥ûý'ç?âN¢?Zˆã@ÚýA‰¸%?î†@áDž»¿âk
ÀMb‰¿ê

Dý`¿êjˆ¿¬¨À¿ÝAÞò"2?r<TçZdAGNbcuTXS 1316+665?ïŸÝr¿¥à?€'3áfAs?dÊÿjØ´?^v"ŠeEM?'֐;щ?~ÑÅ`ªÅô?îõÒI¡ó?›Ú%imÑ?`]N
?k	âÁpêÈ?Ÿ:è·ËÊ?™ÿ/¾
-?íÌFde+?'Å="	¹Ì?‡"҂V]?{M'J­†?­rå.Gª?¦èiV?ïs9æS?ybKðeL9?oò½Ò
÷™?de*ËU?‹CP}í©?u¼0;°Þ4FGL J1317.6+3428?å`ó¹~Å@T0Åë1;âÀ9ʵ™ª`'À<jz4y"P@yáäáìo@÷
=p£×?´Qbޜƒ?´Ñ^¬ÞšÖ?üëNbc¢g@Vð|ªK¿Æ!Ï4`¿å};?HÜ¿æÔXÖZë¿å¡ŽàØóL¿í+™
þ`Ä¿ïâfê%xAGNfsrq3FGL J1317.8+3429S4 1315+34?ïÃ@Ý(?‰¤J<˜Ç?Uâ"…[?VLåE« Ì?xþw™ì‹/?‡Â·1*õ¨?3%"?†½²ÃÑR?J°‰:»4°?`ιô,?…ðj¢óFk?…)áT3×?ïæŽÈ²®?‡®udT­?pž%‰‰	ì?^ޚä}Q?™¤Ä‡gÂ?†	¸¿ÀZ?ïÚäÈ`x?^vöøÆ·?bÂÕ!<ô'?T1OE¹Õ?bXšb'z?QÐþƀÓü4FGL J1317.6+7450?Ԍ°ú«¤«@E<³åuÀ;'mÄÿxòÀ=ŽVox^@W"f1bN@_^4h½?ÏÇíÕ[È?Æ(t"OÓ}?íëù¸¾"?÷õ±Ím¿±â˼¬n3?à:õ¿ÏÖ"î9.¿ä©L•£¿çë@àðÆ&¿Ó~/?‰AGNbcu6C B131714.7+750402?í¬i¦'~~?¬>ažíÛü?†Š0aEã¤?'ÛðՇ Ù?¯–Ù~–ŸB?ª¿D:‰9?î…BÙÄNÚ? ÙÇiµÀ·?w¡…ýB?\ÃQf1ê?¤Èr/ŠR½?œC	Øëó?í	‡zŸã?™æÞ¤qõ'?"ŽÑÆ㢁?ŠaC†°¡?²"çRrK?"M…ÑBI:?íõÌòìR?'óOö&O
?ž	^2©^–?Œ¿­RZ'¡?¡žw|‹¬?…s@ºÊ©ÿ4FGL J1318.1-1740¿ä=dSÞñµ@F]6Þ¹^[À:º¸ÌdÈÀ<fèQ'N@ìË]ë@þÑa‡•?È~ÓD¶?·—
ž¦Ñ?í;Ì^èã@¡ Lü‡û¿ê=G‰+M?ïëÒá长êÀ|1¿Þ¼ŒxHæú¿å)+<Ĭm¿ïÿóÖ&ãAGNbcuAT20G J131808-173536?ï)«Ðÿ?"'n^\R2?gõœ1¬Ò"?iìV¸\Z¼?—ËìY0EØ?"`F1'G?ïh(Sˆ8?"ùòU|¤è?S®Mæ©c»?a­Ëc
F?'À°"b×?"FuÝòŒ?í¢«ÙøÔÁ?•SՋ
Šˆ?…c™ºT;è?veU¥¾PÑ?°>-øîҀ?'n)Súi!?îœãt8?"ùmº<lõ?†d¬8SA?qÒ̵Üø? ½¨°º?¯D1+Y–4FGL J1318.2+6754?î½úü#ì2@H±Ù+áÀ:âñ#ôÒÀ<ö1ø .@ʁðÛtÛ@"d¼B;?Ä+þNå?Ê'€EŠ¤@aãðÕÁ@Ÿ
qÈð¿Þ˜L<™Ž\¿ÑëŠ<¯]Ñ¿äiü¾, ¿Ùº?–më¿ìE ž²´¿ðAGNbcu87GB 131701.6+681031?ì¦ZÓs	w?ÇÈÕmßÕ?«6áÃËï'?º´tcù&‰?ªcqy?¹ü÷Å3?ï¤T†Ä?…¹OØ,K?A™|xr=÷?U…y§š±³?…ÑF¸qêö?"ÉkÊg¯Œ?íÙ¼Šûµ·?–A4&?'³iURQ»?†"¨'¼p?©Š'¥›{Ÿ?'¶ÚÂLÏ?ïã{fL"?V1Ì¢~!?Qì/‰¬ro?A£²`UáÍ?cŽ'9ÝA?R͇³]äu4FGL J1318.7-1234?䆈jûª@HÞÆÞvB|À9ÏhµËÿGÀ<BÛ·K[H@Õ'*g@'Ú˜gjr?µ¡N›Ä?²²Z@úW[?ühMÇ3/Ø@©vƒ¿èŽ?ïûv=žñó¿ß%ôñ¯e¿ãÚüȼ¿á{lB†Ï¿áÈJÕ¿ìQ›žV—¼AGNbcu3FGL J1318.7-1232PMN J1318-1235?ï­jð]·ï?€BÔÂq·ó?W¸ò^–&O?RÚo-%?m?®%œ¿?Z?|ôXڿ̱?ïl–	UÙ®?h·XÓ?X4A"wü?dù8¾5ßæ?éúÃ삯?ŒfF¦}b?ï·ª?.f•,?k_{-—Þý?Y¢û&?<¹?™Jk@¿?cáŒ!v?îqâÒȹ?ƒÅÜù>öÔ?¢ìD#ÏÔ?sñ'–Æ"? ùÂo{?€Ïó~4FGL J1319.5-0045¿í҈äs:=@N¦ùü°À'À:nd-§8À<lf/	@ؼKV@G@ÿ¤?»L·Ñ=ö¿‰ò'­gë?ÍåÑ*ªx@i?%3?ïü¹>z¿äAèÜy¿æŒížÔký¿áXl"h	Õ¿ïü#!BDô¿ë‡ù(ujAGNbcuPKS B1317-005?ïÝÚ"*
µ?'Þ9æ¶s?_偿©"×?'×$ò`ž?b3ö ‡N?\ý±.Qó?¡>õ?ÁrÕ[×?O+)P¾ßà?eåë-fF…?Š_'¤Tœ?Š•¸x\Ž?ïö‹?"¾­l?O?v!ÞùdäH?rÆ.k†æ?šX¶Ñs&Ó?W‰É6r?ïRî÷êD¢?yVD' ž"?yØùØ?g¯"ˆ?ŽWÅ}'×?tÖBi§ 4FGL J1319.5+1404¿Ù=?Ë
ïŒ@RؒyèÀ:Ó!ž¶9À<™>ÔI™@øËagÏ?û߶må·?Ïâ+™5ñ?ÐA´ †å@¹	k¹Œ~@v®óH?é¬
¥0ç¿èæä:§›»¿­÷Àkj‡2¿á(ŠÎ$»¡¿Õ/æ5T¿ðAGNbll3FGL J1319.3+1402RX J1319.4+1405?î'ú½°ø?¨ù
z®N?hçE·Hl?a'èºáP¯?¥QâÛI{ô?¨¯¾àò?ï^×?›"Tƒüº?c?±Âpœ?v	áÐbω?›L.ùE?™',FÐ?í0t(—uv?™Ì›§'??‡Wþ[+?x('œs9.?³šS»Èê?—šÇªå2?í"ªÇYë?˜Eˆý^(5?€u½æ*?qÏ8£µg?µ‹Kò"Så?—`ñڔÛt4FGL J1319.8+7759¿´Áç(÷"¿@C"{¢7ÍÍÀ:)6&,ºÀ<ªÖR5W@¾Ë$V ž@Y©qÛ?²"`_;Ná?Spaù.@
‹éû†Éˆ¿åÐ!ÙC©¿Îd"i®ðC¿ä΋魮$¿àU<þ
6Ÿ¿ßÐ`zn±¿Ö Uu}ZŸAGNbll3FGL J1319.6+7759NVSS J131921+775823?ïóD0únÁ?X¡.EÏÚ©?.o~niˆ?$ÿüë÷¥ñ?U©®=^'¯?V°0úš.?ïµÿ`D
U?£èyô8>?<¨¨|J/f?Kä©Ø*&?šâ«Y
?€»L(¨Õ?ï=&†h?~±x,Ñß?d€—Ttã›?ZßdJ캁?•ËHpÂP?{øz7XAä?ïÕÓº4?\:¿à&s?R·´ŒÔËÌ?<D?‡+Þ?pɉrí²à?Yü´‹B`ƒ4FGL J1320.7+3314¿ï™Ìð3.V@TM*®)s—À:ÖÛÃ	ÕlÀ<€ëLê"@êØ¿IV‹@g†
¢?Íía—ÊŒ?Ò±×~¶ß?ÿi±Y©¿'@(¡ ¤$ã?ì†X>…vÍ¿åÎj[¾l¸¿å­u"›Y¿ëÞ`]Ï·¿àù«ƒ¿ïÿÒþÀùAGNfsrq87GB 131814.4+332742?ïHC©zyÊ?¤1|7¡'?g=­k7ª?hºin'_?"Õ0C_Ÿ?£ú …F€p?ï…þ‹æ?¡ߘ†s˜?kCúÆá"?}h=CVmD?›ÀìÕ¦ÿ?¢×o°4?íjŠÉü3T?™
¾²ÉEp?'܆•5
ã?"—úé¹~?¯é¢E\?"iÞÕïáÿ?î~êÂ9?:}JìáÒ?®æåöj?r¸Ûê?£¥Ú"Ú^Î?âXÈmü4FGL J1321.1+2216?çÈÞµ54@Tlºˆ&«À8ŽÅâÍÀÀ;°…ù©¤ª@ï°¨ÔÊó@@gc¼gû?¤)0N&v?³Ú6lΊg@Î^'lVj@rø_¢¨¿ÕÚj$"¿àđ"èYñ¿åG˜_ݶ)¿åž@ÈG,¿èÞê¦ÒgA¿ìJˆ_	¥ÆAGNfsrq3FGL J1321.0+2215TXS 1318+225?ï¨Ã'éš?€@AÅà+?X¼´)^i?X"!úWé?'·‰0ÙÖâ?~Ì&Ã,×R?ïwÄØ_Ü?'RFB|?Y0¬æV3s?uïSübî=?Žè´Kq'–?!†\š¸?ï¥×,Ä?†…꣢1?u¤¬÷¬ï?kˆÈóÍz†?—@/@?ƒ%{´
?ïå)fû™î?W¿/7äé?Iõ¿æH?<ð%q@?dYVl€.?TËG´4FGL J1321.3-2641¿ï±.€Æå@AØàÉÙÓFÀ:ب)À<L[œÞÈx@bó•8Œ@;þ¦c¬x?ÀªãƒrÁ¿¶B³-êI
?öª¼¤¡5@Tä©~>¿Ï""ÜÉ9¿é1àþ¿ì'ð}V¿ŸPg˜âÜÑ¿ç ÕÍýNu¿ï÷ŞÛ!úAGNfsrqPKS 1318-263?ï‡Êu´n?‡ðL#.úÔ?u:á¼?rìÁ):Š9?ƒ"Å!úœ‰?ƒÉm¯…p?ï:xŀ®®?—£$e){Ú?cÎð¡…ó?yc5«Ú.?–7%±Õù'?"QÓýån#?í"%ñ¾©?"à‡_`Hÿ?…Jý@GIW?uáÇ
T<¥?°µpÏA!Š?'×ÃL® ?îJæuC€Í?—HƒÔߛ€?"~o‰ùœ?€\`{ê!/?¦1üɃ´Ý?"ã©]–4FGL J1321.9+3219¿è–"tˆà[@Teˆ±Ù+À;IÀÜԁÍÀ<¸Hi%]ˆ@»Fc'ŸÐ@À
¼%/?Ål¡«¶Ó¿–[߂d§R?ÔÌÎzKö@ä*m'ÓÒ¿åV…þ\;ë¿äæœau÷¿çSˆ]‡º¿ÝVÀ	¿æ\C'‹¶?‹›Q:ìKAGNbllNVSS J132159+321903?ï5pG"6ƒ?"'˯_‰?QÈR¹þ?GÚyU¶•ñ?˜5vˆmÈ?"É£@†Þ?¬(L'?‹†³[>ão?E×yÒ՛d?P˜Àðv»?ŒòÝX¿…û?Š•¼òÚòà?îHWdHš¬?ï–öó­!?qäSšúÙ?`1é—SŽ?©>Qõê?ŽF	Ùü?ï%T<ÿžh?'ÒàžÂG?dy Îã™|?U§ïOÓ?˜ÆTF/¿Ø?­è7Òb>4FGL J1322.0+8317¿é<aÖÅÛ'@@ã×<'W†À:\Û¦"c§À<@–ÉÁ@!š…Ò½R@èJה§?Á<´ÿ?Á¾z¤‹åý?üà·õ¥3@Á?à뒶?ã;xçrj¿Û®qÊG·¿æžÍë°½£¿àÁJ³οëù®AÇJ­¿ïýR†Q¾AGNfsrq3FGL J1321.7+8312S5 1322+83?ï'-iˆV¤?™ÉãÚEð?fߑØ÷Þm?q‹ð~I×õ?…üÁ'¬^Þ?–zvŒK(?ï®_ò–F6?Êöûõì?C²Ö!m*ß?X,çã­|ß?ƒ,ÕøWŸÎ?€K¥â¬&â?î¬]¼J¥I?‹!·kÌ
™?…B´ÕX?w˜¸2×? Øã*¨v(?…ŸÆip¤?%²?eÁt‡Ål?`ØGr‡Â%?HÔCŠ*`?yQZ=bØf?cbN
¢°n4FGL J1322.2+0842?åðނŠfÿ@QŒ2 f<uÀ:gég7F¾À<~ˆA'O@k‡}'@_`'÷–¥?¾&4ÈÂÇ¿—©Ä—ÌÝ?Ú5˜}ºÀÜ@"{½™Á¿Ú¯Þ|·â¿ç–œŸ2ŠÂ¿â.5!õÉ¿Û:…M\T¿ìrH½3«¿Õ±$ûŒÿAGNfsrq3FGL J1322.3+0839NVSS J132210+084231?s®üÈ?¿7SX?c ,\ïº?W 0jhT¶?…ý>Ò:?€;$*ȏ¢?ï¹%о?ƒ¨"Û^?:ôF{ž?P
ú3^Tï?€èW÷–?'²®)öú?î°Þ©dP¨?Žï‡îÅ8?",¤z´?'Ô¼½R?ŸÕ =#­Ÿ?‡ŽæQŸ­?ïÊ4ó;ù¨?aÒþ—£?Yx˘:?JÐ1c õ?t‡S{ô¤e?^¦¿;@î4FGL J1322.3-0606¿ë_×"ˆ@K÷²VÿÁÀ:óY'BCÀ<´¡õˆ­¹@@ ?û4ï*Ŧh?ɂ§Í"]?Ö¨B¿BJ¨@3å	Út?ÿl¿y'3¿ïÿúVrÓ\?ïÿêњ'ç¿Ô	B%¿ÝjwØ~±·¿âYDàá6¿ïý'Æf>AGNbcuAT20G J132219-060619?îU'92&ê?YV–[7&?›¾ÈÓò¥F?'ï0È-¯6?™ðÈ}m?"ªw	åù?ì\¾}Ä?¸/?¸}+5?¥hž¼5O?®n)²ïi?´ÈÊ­÷7¤?¬çòÈԔï?èxÜÉ ôm?®WéS*×?½ß¬¾¿?¦þñL۞–?¾Ylø9A†?¡4²"®˜?è"/*1Qd?¥ÇÜÈэ?µ(­#>yö?žm1Àç?Ãìś}u?¡`Ð\©-N4FGL J1322.6-0936?¸gûíÅÂw@J?^g"dÀ9.ø6#
À<"*M±c»@SoЍ@'êÓ²š?­Š¿q6	?¹¸A¿+é,@û#š8ûÊ@«AOÝ8¿´"ôxA¿ã¦¡Ÿ¢r0¿é,.âkšƒ¿éŸÎ!5¯º¿ç4R¿æ@Î&i UAGNfsrq3FGL J1322.8-0938PKS B1319-093?ïÛÇþÞ¾¦?™‡Ñw²?BùkõÈŒ?ov-Dön9?oy¦#ÏVq?•ž›¡&úÏ?ÁsjI?‡ìq*Œ,?D®Üâ³öu?XG/D
™?‡O¡Ôú.9?†òú½"U?ï}†ó>‡?ƒR»[‡Ë?q%ú]d­K?iš€M›?˜fЊ?æ?Gó<×îg?ïö™öá?B/B©£ÆÞ?3¶æ¯§¼‹?%Sq¶Ö¸Î?K¾"̧͕??Ê##ÄF4FGL J1322.6-1418?ïÝTovŽ@Gð*#¿ø©À;wëÒK'ÏÀ<°$?ziS@ d°êöY?ÿ)¸`.>?ÑÔȄ=¼Ï?Å´!ZBÁœ?õGuàVíM?ôí¡
Ò
¿ït†ŸÁÑÇ?ïüÖ 
L	¿âL€ Ì©;¿Ý3<mn˜¿äô'Þ½¿âÍÐØËÑAGNbcuTXS 1319-140?ï­_·Ä=?®ÜŒâÊ?Vȱ¤îñ?T–üzÝM?å¦ûÚRá?€ªgÚZˆ?í¯.Åm–?­Zî@"J?‰¹¸üYÄT?'À|ê¨Ñ?®ž¨Ä'µ…?§N]Ø¥j"?íîåa:¹ú?'ÄœÕY"q?1µwBêQ?s"&@ä?¬Å<Žƒ¥­?Úí^óÓ0?éˆdfÑc¢?§'ãµ	öú?ª÷BϚ?œ"@!•?à ¨"Šô?¥¼DVzv4FGL J1322.6-1617?íL%$9É@FöFñVÀ:½i&4G/À<€SM"î@FÒ̖5?ÿ~"ÐÜý?ËÈÕFmø?»@ö•H&4?ñ%HĔïç@QÉc?ïñÑ~N³¿é§ùä]K¿à/÷¤ç«¿Ödf[ÿ…1¿ãðý=ØӖ¿ïÿøãúAGNbcu3FGL J1322.6-1619PMN J1322-1617?ï± G{‰|?x"G•'&W?IË¡Õà†?B¤Îú(Åk?'ñgBÕ?w\¼W{$?ï6|¥Š[ç?[78L-?Wò6ʜ¬?a^¸Z¤»J?—±Gí—Ù??Žíh_㩙?íðe˜n;ü?'?TˆŠ2?vִۄ×?a.ƒÿÓTx?®6k¢€Ï³?÷g îà|?í†CÃÔ?na"âLŸ?‰dhÒ(~®?sGêÿç?°¡VלO}?Žê¶‡Ïp4FGL J1322.9+0437¿æQ7†ÈO@P'ò{xÀ:ïùwO¶À<™€TN5î@ L—ú³?ùnˆwÆ?ÔCÔýKp?ה&}˜1:@2äÄ:W@ʨ<ʋª?îÜEæ"0¿ìõ΃†1Þ?Ïb`\â@¿ÂôƒJ!â(¿æ5'ST:ë¿ïñH­ûŸAGNbll3FGL J1322.9+0435RBS 1257?îz åàc0?¤Q1ªöæ?f…SÞ ?eq¢ÎñE?¦ôILÈ*?£òùŠ',?î¼ÇçÑMF?£%•XãèB?pÐ~'k‰?~ªº·'O?¢€"þ<?¡y×­H¹™?í‰7ܺw?²Ê1'g?…'ôv^?tMÍ$¶Ž?´«W²Y©¦?œ°4‰9ó?ì-hˆpF"? hÁä‰_?‡L¶~£3?yg»¿šøù?»«$ì©kj?ŸÆ·Gµ¿µ4FGL J1323.0+2941?'à~aX*@T¦}¿H€À8è[;ùÀ<ʍWkø@9Dü3l¿@êKáQ?¤p½¾x1{?«²DœxWf@œÄÇDÎ@º`@²w·?Ç2"åX¿ßð(‡ƞ¿ã½†]ҙ¿áŒé½ž[ ¿å>¨²;Q¿åwR|¤–MAGNbcu3FGL J1323.0+29424C +29.48?èëdÜ&è?½zt²ËY]?"ÿžB­?ŽÏ™ú,?É҈¼9\?¼t[¤XM?êçÄï~?Æq²ƒoî?´ñ&˜SH}?Ál&Å@é.?³Ð¹X0Çx?±±¼jÜø?é{éChÍ0?«J¹ýþþ?£в<w?'8€6a—í?ÅOfŸ¼?¨»%Ùhkþ?æÞ	å÷ñ?µl*bÅâ?Ê÷
4'íR?´¸N~[?³!–g!íÙ?˜†&§ñ4FGL J1323.9+1405¿¼wó&þœ@Rº×à&EåÀ9æO"}ŠÀ<3PëªÞe@ cøÍܗ?û9AŸÝ€y?¾ÏiŠ2H}?Á­wÝ\<@í†"ÄP'@¦©øa{?螺¯ÀLŒ¿ä—P~"Ñ¿Þˆ…3[!¿Ïñ[øNZ׿ޠÁÁ€éJ¿æ/RY,AAGNbll3FGL J1323.9+1405RX J1323.9+1406?ïÄ=÷"ïg?¨;†‡Áœ?sRû3 ¿	?¨L¤¥Õ«?eÏ\?U·*ݬü?ï‹ðïU8?ŒJˆ·j?NöܶÓZ±?\7­^çL?‹V_Q¼?Š½oì,l"?ï­ß^
?ƒÍ!´4Xê?k&·"3s?`T»zÔ¢¨?œ%m!Ø?Ä?'rI}8'?펅¢	£?šö€ð?ƒf?»±âv?nx†èóÆ?®Ê—¶òí)?Ž™lgLô4FGL J1324.0-4330e?Ñ¥\QJ܃@2ú&€IRÀ7®Í™{f©À:ØÆ;¹²@D*Se­¯@Äw¡!MX?£®¡†­?´-2<@à
quŽ@ô‰PKFû¿Ú=1cÐ4
¿ä+ïý©c'¿ç9m	Ö¶¿çÓÞ¿=˜¿è˜—;ˆ¿ç04{1ÐAGNRDG3FGL J1324.0-4330eCen A Lobes?Úâٖ¦b?ÆÅLµßoª?µpŠ]å§?¯Ôm›'…~?àMàèð?Ç`¿õ…ä?æ+-}=ô?Ϫ¡Iw=?ɐï&ÑÉ?ËÙ0B> ?»…(UÈlØ?¶¨æÛl!V?ßèù¬æJ?µ×[Ùa?¶[Ãمë? ¬ ú·z?ڀêñžõ?³aa"	."?á†–×NÞ?¶át¨íý?Â.j~ƒöµ?¯\Š,{V?Óܱ"fè?¸ˆNŸcmé4FGL J1324.9+4748?ç)ê™çG@Q³AáKàÀ:A(Ñ°aÀ<lÖ#£Â@+»öÀ'@#ˆ?¾äaéÔð]?¬PÑÿ'›?é"x¸xò@aŸ~àÛ¢¿Þ}³¿µ¿èüØÎbÏ¿çtøÀEªÚ¿ç8uý³¦¿î'âJãS!¿ïýNª‡þgAGNfsrqTXS 1322+479?ïîÇwTW²?h†œè——­?E2‡ËüßÌ??[½ø¼±³?W×ÍqR,`?fä%À»ý?ï³ù·´c?"ƒ–Äñ+÷?=þÜU'2?Qê%25NÍ?'Íû0:t?ƒ—²œï³?ï/Hû>Øj?}r}­/$Y?o_ÕR"ɇ?ZcÑ\±ªo?–*åíÒy¡?zœDl†W€?ïåjrÄË?VÀÅZ=–d?P5NPcF?A|ŠÖèŠ?bzæPó?RÞp¾›Ð4FGL J1325.5-4300¿´ï­S^¤@3k8''À7~'æ!1©À;H4[Q_n@@`MȊÉ@:´œT^ý?'œÅ+	¿¨*Àüg£@‡0ž-}@!¯Påö"¿Ñ{%û'2¿çqÊÛ[¿è½*BsÂð¿å½Ž€á¼É¿ã1?=,±9¿ã`Æu(AGNRDG3FGL J1325.4-4301Cen A?캷ÄZ´?µ6Q A1?—ÉH¯åÊ?˜Så·»éï?´7ï³Iðã?³à5*4?ælúÐ
6?ѓ÷¥œã?ÉΈ*9?ÏèN±'U‹?¸üoZñÔ?·ý
@¦iñ?é<
ÉD§?®ÂäÏM
?©ç	ʙcM?šzÚ¬Þ8?ĖhI?©Žÿzü?å4-4WÌ?º¨Ü–d[?Ë÷lô{0"?¹\€†«äÇ?¾o¼tM0ž?¨*_£Ñv4FGL J1325.6-0227?ꊤX&v@M¤Ù¾L×IÀ;$­‹¾åƒÀ<¡Š¯@ q‡^Ù8?ýªHiü?йܚ )×?րB¸â4@Á	š³u
@,DeN¿ïþ"ƒÕâö?ïüA™þCg?èFp¢¿ÖµÏÅ¥'¿åˆqy‹¿ï²!…‹ÅœAGNbll1RXS J132542.1-022800?ïAPŸË¾?€þ	=û?~0õ¸-¦?tü2:F©?I®˜|þä?‰¯ŽœDa½?îz¯Vd?¨T58	q?"{Ú÷Ÿ£?—8ô_…¯?£9
"Ò»? >ü®ã?ìŸp¾ª¡? Cm3_–c?—+î5ëg0?‡j^8cS¹?µ9~''Ñ+?›3§‡??ìS³.Aþ•?¥ý…ÎÌ"}?¥3¥ä7é?žõdía÷n?²È"›îoh?ì§Ø,€4FGL J1326.1+1232?æ¿í"O,°@RRwÄ\»ÃÀ;p`B_öáÀ<ÁîqbBë@ ŽG¯—í?ößùµc#¼?⧻Ðüv?×k…òž?ù!¨¬\ý@]cIP€÷?ïé`p¾.¿­Æñv–¿ê˜¶zzða?Àe­™UÑï¿Ó
Ÿk?¿¿ðAGNbllLEDA 1410672?îî›{hÎ?¡—<?~M ?pÜ<NKç?z{"D+Ð?õÝSs? †Ç)x‰?ï]Ñ-su[?–*ݒ÷—?Z‹¸!?qÇsŽh;I?'Ð0Ä?"É!ŒA¡m?캺¾Õx)? Â-œ1GM?‰ÃchØñ?yéAVå-±?¶ñ½§g#Ž?ŸÎdXx°Ï?îr^BhÂÞ?"./Ç-8?aû…¹PÉ1?f¨ô¯¸êE?§ºc}ÞŌ?".PhÏ»û4FGL J1326.7-0503?Ï?TeD@LXÅCk›À;ÞÈè;¾À<×ÁЈg@"æt™Z­?ù2Æ[™ƒÊ?××Õ^Á¬]?´ìU~6¼«?Ԟ$ƒBM?ÿŽÞëuj¿äÁ@ýv8¿â¿Ýѿ恽¥œà¿ËbFÇÇÄ¿³ØDЩ*¿ÔLw½PØáAGNfsrqTXS 1324-047?ï89å*†??'¼bªtõ(?FT¼¿ÈX¤?=)¯À¤?˜Ft°õ9?'…`õ4\?î :­#h?ª.@탗ù?j v¥FŒ?~õy'Â?¤ZMÅ)`Õ?¨0Ks[Z?í«ŽEÌ®¿?"æˆ,üq?p£€¨m£¸?^ùºÿ¾© ?±™UǯÊ?"Zœ%Êöˆ?ìaóÿ"?©Ù­ìÊ??Z¼Á}G?_å¾Àn–Ó?¿eýZ??©òzcr»A4FGL J1326.8-5256?ì´óʒŠÝ@#ÀL‹ÉÍÀ8"¶»éÀ;\hÑz±w@¡×sï»å@mŠaî1¡?©9è?U;­?Á ãd鹘@ÂÍáŸÂ©@ЯE¨UÊ?ãýߔO­½¿ß*ø…«¿â\¾™XV¿äsY(B¿é€ÞLQk¿ì5Þ>XˆAGNbll3FGL J1326.6-5256PMN J1326-5256?í´uN=Ë?£B@aí?qÌWeψ?q€¹cŽ'á?±?»,?¢¹I\ýse?ï\|áEä?œ"0«|ï0?Q".uälN?eØóiöÙì?"W æ¸ü«?œ Þ¸¨#ö?í¦íJüžz?žûvµÞ4?•Ù­bw?ŽùMn°?ª¤ù"ÜÔ?•ÛÒû(?ïlÄÙsz®?z°ëöjîT?Z·ßӋ×?LF?Äû?»æáCqn?yWßàÈ»4FGL J1326.9+2210¿ï½À"x¤@T"¯ÌáłÀ8à~֟´fÀ;ÌËQ¢Š@}YÏT;—@î,ëñ?§›¶Õ>¶I?¾L`RP/@]"Äm'º@¼]*}'¿Áç~~á–¿âYÏ^ø]õ¿æåÂ!M,¯¿æçÁz‰3¿éò¶ÁG³s¿æîè`Q#‰AGNfsrq3FGL J1326.8+2211B2 1324+22?ïœ>x³\?…7eÙÒÂ?aƒêq¸‰þ?ZX³c'ø?"€eŽ?ƒà1ÿÿâg?ïoIÔ¾wÓ?°÷ö™h?Veuï°ï9?eîâ²dwL?°n	5ö‹?³Ç*±"Á?î鐬¶;ý?Šžôåæ–?z&gë£ò?q'D?X†"?œDJ=—?‡Yúqf?ï…ÚƗ×?tg]¢VéV?q ýT -æ?_$!e5û±?…øþ$Ió?päÓwLX£4FGL J1327.8+2522¿ãì%²ìüÃ@TjGG"#À;¢
6Ih)À<ÜS'ˆ@!S `Q®?÷_›ªcì?Ú±ÜÜdok?Äß	$ìÉl?æè$¬‡²ç@ßbݚÐP¿åJ›ÏÔ¿
¿ïÔ~ýŒ`?ì?©-‹S†¿ß7ÀÜ~œ?"?QyšJÄ¿ãX^èm½AGNbll3FGL J1327.9+2524NVSS J132758+252750?îZpB«ú?´O.Lês?`zÔûŠXy?`k¦W秶?©QN<šã?³ô}_"<?ï,LÝÂØ?¨E›ûx'?Yÿ%PŸ?oÃiÉ^3(?˜Öq÷\oí?§ƒN¾È?íê3ý? ²á=HØ?rOçÚk€Œ?bO–©ƒÕç?¶«¯âqË? †6X?ïî§^Y8?:#Î{?%ô¬ÔwÉ?,ÒV:žõ?ŸVAºŒ®?ŒçÙm«'4FGL J1328.5-4727?¤4çr¨YŸ@-ã
£3vÀ9tµÙk@ÁÀ;ÀŒŸ5@ áWÕ©ë ?ÿù6Òúä7?µc`øh\
?…³'Eæ?Üój:±VÐ@Σü¿è8ÅÖՏ?îAdÿ‰¯¿â]"Ð_¿áPj¡3–Û¿Û®ˆ^]ÙO¿ØVÇaþͦAGNbll3FGL J1328.5-47282MASS J13284063-4727496?êÝwe~ƒ ?Ҏ=HÞßÕ?Vx¥Ò¹"?T)Æ,í‹~?Ä^xºL
?ҕ>-‰ïß?ïzqþ¨	â?'jkp.ñ?R§ÃE''?bÀî¸L:?‡íM5W?'d}¯(p?í}ƒÜñî?œÕ$°N\?ákb…Á?rÇú~.²ñ?²#يbH5?š€ïò«ý?ì úËdÂ?˜qÀçYèÄ?Œà¿Ó~/?x7‹K7F?·c/5
?—ú¢4ܹ4FGL J1328.6+1145?ËÕí4×@R¯_Ô{îÀ;q3JEžÀ<¶èÒ¼ÐÖ@"&6oÓ¢?÷÷'#'?ÔÖNád‰l?ÇðZpŽÞU?ôÏsÀÁü@©_àˆ¿Â¸G"£é)¿Õ¿¯'ä÷;?Àˆ]¥¢'¿Þ=—$Ê9Ê¿"uUËFò¿ØY9W9£AGNbll2E 1326.1+1200?í9щÕ:¯?³5­¬­s?uöTà&ʾ?o~Áœñ5?´ÒcS½Ý?²ÈMÅùöf?ï8q$Ù¬? [86oÉ?ao'úÆS¸?yd	xà]ò?œJÿ|ÿë?ž:ÄýÁÿg?í"år×'?•ãèk†°?zÜ"wÞ?kùᔌÅ?²+?mð?"F>]Dq?í¬~ÛL?žCð)ñ…t?]ÈV™IƸ?Yjۈ¼N ?·{zµ3þ…?ž(3ˆÈé4FGL J1329.0-5607?îh¬º'>Š@y bvÞÀ7ÛjUß/¦À;ßTŽÍŽ@ÆCß}Ôl@Ì=s(? ;~.ˆB?½±•¹»"*@STâ°cà@º•¼?`é¿Æëðÿ\+¿áŽ›¤5Ôοå‰AAé¯\¿å¤º|h¿ëË7×âr¿åÀ~SÂöAGNbll3FGL J1328.9-5607PMN J1329-5608?î<֖ñ‹?¡pµÌ²ó?{ØÄ"h6W?{cÇ0Xß?¨·~šGù? 7×bìUç?îˆVîks?³½H±¦ÞY?aäÓPÙJJ?uȘè}êÝ?¦\Cä;;+?³oþÐ$ì4?ì½U¯DÅþ?£ô™ƒá3?¦g³¡Rak?™ÉOMW?­Âñja>¨?œ¨t½vqp?V!ye?v·}]'"þ?W-…Î%yG?PŽ·ã~Ž?…ô¹½Ü÷‡?u&ò⨡Ã4FGL J1329.4-0530?íü·Øì7C@LçáüúÀ:¯'m-*À<P*º¾­O@§/¬@ti
à"S?ÉAV÷Þsh?Û£Ñ@yí­@ö¤^ïy ?ý¾£»º¿ï6¯õ%±j?ïæC_¿Û1W{fþ'¿ä'–NÜÝ¿ëFQˆˆÐ¿ïÿŒÝÉtSAGNbcu3FGL J1329.1-0536HE 1326-0516?æPÛö¿ç(?Âô"¾"?É=˜U°U?ÁJ³AüéY?ºýðEUf?±[Eïé±ã?ã7Q]Z?È¢}MI]?Ð]"ÅÙ£‹?ǘÑ7£·?Âhu,['?µb%ëè?ãˆвX_?±'#m¿y~?ÅCX¯f?¤ð5¾pQˆ?˲Ñe)ï?©ä)øfJ"?ܨfÏמ?±aN£`y?Ø\
12­k?³ÕÀ½>©î?Å÷ýëi+?£åÑzžŸ4FGL J1330.2-7003¿©ÉbªùÀÀ#éêÀ8±òAÑ[¨À;Ž¯­Uk@®b¬©@Ĥúö«Ã?¨VsÕå¡?ÂéËÎ|z@€èÈ«ÕÜ@ÁÝFl è?ÃÌàÃÏ£¿á§@¬m‡¿æ³˜H`¿棖b'$¿é,Ân¤ù¿ï÷`Ÿ'".AGNbcu3FGL J1330.1-7002PKS 1326-697?íä,€!v?¢^θq?|"dEXñ?y§•|7Ñ?®*Ëu=•&?¡Kv¸$,?î·\‡ó?©ï,êç=2?<fk°I#?U¦ùî/L?¤Qq8VîÄ?©É ‡j?î‰+Æ"E?'¥v'{iU?"ªòº¨Îs?~ðö²äbR?¢B†ï5˜
?Ž›Iðâ?ïÕüšî¿?bWzQÛ?;Ts:¼Â?0àã{¯`¼?sLkUU¥9?ax†>öæp4FGL J1330.2+7002?Ó›
÷™™@G\xB0üøÀ:S¯Ã§ŠÀ<µ"Î~}´@BÊáæ'?þ2‡V ö…?·ê"ßph?°Ý'ýuâ?ø^–ÞÔ6N@
ÂÚq{x¿çéƽ¿пÞ'</Ü¿à	¦ý…Qc¿ÚÔ¯DP¼Ü¿â{Ó {‹¿Ýx"á{°{AGNbll3FGL J1330.6+7002NVSS J133025+700141?ïêO$Ë?l¶ì;Øê?6A»Â`™J?4V«¾D1/?c²8!Ä?jîM)§—¿?ï—ë§õ±ž?‡~Qh×F™?H½Î¼'2?WÈ*%õVA?ˆy9Ñ%U?…þÔ¿wÓ^?ï=Ç:&†?€09@"n?e;"¤Þ"?bìÍ+ñ"±?•Ÿ¦)ß\–?~f€>á`?שׂ\"S?gñÜú~ð?`«Å/¯nÓ?Gû-g°þ?€ªGó"?eڞ¬ƒÏ¼4FGL J1330.3+4441?á%˜Ýâ@Q²–»˜ÇãÀ:qy¶ViÀ<©-óXQÑ@`;€^µ?þ˜DЩ*?¶ÿ{?Áh§HÙ¸™?þTuˆBYA@u>Òx³E¿ÝG"Ô@_¿ØEL»D&¿Ü⛠ÚÖ{¿àF@V1dý¿âù|"MÀ¿ïþËê'QAGNbll3FGL J1330.0+44371RXS J133021.4+444117?ïŸÞðk?ƒqç~Î?loõìA^?fl%['‰n?€ìF"ìŽ?40®¨DW?ïFÃïhSù?"1a É?b[Up'ùb?mR¨&?"Üdð®?'p¶¦)<?ï@?[ ä/ÆP?'i¢GA&?uÒÁ'z¸?©züM Ël?Šk( ²z?îìmïWÜ?Š*\âÇa¼?•5¦z˜ò¬?|X3Ÿœ3?£veã¾ó?ƒK;[!k"4FGL J1330.4+3157¿át[Ȏà¿@TêòRÀ;q–EQCÀ<°0Š‡@>u–8Ê@A&ÜÛ±?ÎÓʗé@K?Ò÷ ¥U@R]šåÉô@ÿTWÆ™?á拺³Å•¿»Ÿß?&l·¿éÓÛ·lé¿ßâWcJ¶¿ïÿa_3¿ÞP·þ^•7AGNbllMG2 J132953+3153?ík6ÿÉÍ?°Ô–Ã0 …?¡çŠ=kÆ?ž7=>DÂ?§eѝC?­úv:þ-A?ì¾ÎIÚ?´­VÎ	×ì? ×ÓnÜO?§w	Þ	H?±£gÄ?«Þñ:/ð?ê[‹o'?¥)i¯G¥?¯vñ$`?–³àÄÁ΁?½"ìž‹ñM?òœÇÝÜ?ê–ê2'©ñ?¤Aæ.•ÙÇ?¹ëÝ÷˜?¢3ó7ޝ?±]¨XŒ¸ä?'¿ùd—×4FGL J1330.7+5200¿ãÊ¥à`@P½çXÀ:*q?|ÌÀ<€ç"øoé@–A»6Lm@'"4H?·ª4??¡±…c°?çsqF"9@ùP¢"пæ	—Xv¹›¿å	Ý.Cà*¿åC‡sý'Þ¿ç•žvx,¿å'×="
9¿ïùía—ʍAGNbcu3FGL J1330.9+520187GB 132842.6+521750?ïŐ¼ûH?rŽûE=?SºQYûk}?I!C(ј?xIkK'&?q)˜CD?ï{#í¢¨
?ŽEeZч"?QxžL%³ð?a€;ª<œ1?ðÍÑFÒ?Œ"zl̎á?ïb¼R?.'‡ÿíù?ki"‡Œ?UZGY­6?˜ÆŒ7úd²?S½‹%ò[?ï;ëÎܵ&?~Ǘ›«š?:¨bYw?löÁ;!Ç?ÊcæyŸá?y™IHƒÔ4FGL J1330.7+2933?êš{ÇÕ@T@ò@úœÀ:'ßBñÀ<…0¹o¬@Êiïۛ@›Û ¥&–?ÆšÍ Y¼µ?ÑÃZб@œT\È@H‡RŽm?ìs€àæ	_¿Õ]ê–â/5¿åÑu=™¾ƒ¿ìTR½'M¿íÞæÀ=ó+?åYã¡$¨VAGNbcuFIRST J133101.8+293216?횸Ãlâä?ºW¾ÝcÞú?ˆúÓÍq›Q?ˆ,—Ç*ä?°
ßjêµp?¸ñ¢iǽ€?ïZ÷ý,Ò?™lóÒö[?gv¿8½Ó•?…%l84Î?'²FyB«5?"6
Õ©ÿO?ìì/›ô?£Ôa'÷†?£åï2?">?,õÞ?¶"+ç`?G7¡†ÃÈ?ïWä@'»?Wù²Àä?'7—¾m?t·ÖÅk1?‡ÏX='Í¥?xâq¦€o4FGL J1331.0+5653?æ\h2ÃT@M´k&¿‡jÀ;Zw'ÔáÀ<ïcáPèP@ ùŸõÿ 1?öûUvT?ØB·ÀK41?ÒFŠþÌ#?õb¥ç…¶?øj¶ü¿â°›ÿ$Ô¿ê[a .Q¿çp5½Q.Ç?ªÁdÂUD¿ßZ_U¿ÚƒT]ÐAGNbll3FGL J1330.4+5641RX J1331.0+5655?î¶Y¢"'ö?£‹†ž?bb'W'§"?]ÎZ'êè?£t=±UV?¢‰Ï1¢Wr?î¦gñè†q?§±YÞ?l"RbÚ1'?zhàôï??£Ñ;»IõÄ?¥Mƒ˜§ÿ&?ì±!is…? Ð3¯µ?ˆ]^ü"]?z}Ë 2?·kG!ø*?Ÿ$¼
æ–?íxÒWΘ5?™‰¡5ƒ³Ò?vܔöJ?ws=,ÖPC?²Ë¤jî?—ú)|÷z4FGL J1331.2-1325¿î½š8a+¥@H'M3H,À9™X¸'úÀ;ŽŒ3‰M@4@#‡@èŠÛ´ï?Ã>êáà°/?Í&ö9ÔA@ PxË@4j­óò¿ç¬h=Öû$?À‰ßgY+¿æ ¤_ñ,S¿ë`ö í¦¿ã°W¡&«»¿ïÿþøþ"AGNbll3FGL J1331.1-1328PMN J1331-1326?ï}bº‰}?E¨ÝýW?bw>¤Hy?bL´d?Œ'3ó¶?7Ý>
¹˜?î}פ£W?¤Þwúàò?{ª%UÕ©?'¿ZXn?¤À0qÔê?¢½âk:.?êvBÆÕ?ª­±?¥J;4<R?"^$ƒ°ðÕ?ÀÔhºÑÐ%?¥=§'‰‡Î?ékÎ÷[}?¥‰þNU@?Ÿ$å³{S•?‰S'Ñ FŠ?Æl'l"¡?£ë‹¾é4FGL J1331.6+1711¿èõ½B¯ì±@SEbàŸèÀ:@óÖ&À<ptšÐ$@-…àT>@Á]}‰˜›?¹<ÀO»Õ?Æí|Õ¡?Âi;,ü¸@R:«økâ¿Ý«$[¾¿æ1L©%þ—¿áëâ—°¿åTÍ·®X¿åÚ;€ÎÜ¿Òg'áC§JAGNbll3FGL J1331.5+1711TXS 1329+174?íã:Do'A?§tž]uz?s¦T«~·A?nƂ½Zly?¯W'#—?¦ºäz¢iã?ïƒnMvD¬?9âð~bÀ?M÷Ú}ÅcQ?bGB>Ê?Dîú'~›?‹z°'š÷1?í}ë8Ø9e?–½cÉ¢Wû?ˆÓzòŽ—?y,+yý^?°ö6Úìaô?"ŠØ$gü?ï
B±º€? äÊïV?€Oýi
íÜ?k‰_ès!ý?–/½µC99?|±§¹îë4FGL J1331.7-0343?¢?UKÿ
v@LÓ;÷'À:]òœj.rÀ<Õ¤ãc@¾k[m¹í?ùæ(S`'?ì1d™ˆ?æB^
ÒQ?þÛÐ@Ô@T@¹Ù€?åðg¦ØF~¿çQHÇïî:¿ã&ØaU…n¿ïÿèã«6¿¸š¬È®¿î:
BâMAGNfsrqPKS 1328-034?ídÇÀy£z?³ö›j'µ·?z‹‹zõQ¿?'Í:7l?³1	Dƒ?³/™#P#¯?în£«H€P?­ÖÖ
—?€´Ðåƒãç?"ä…•/6Õ?¤è'
?§ÍHm	?瞊Ì^ºÊ?­õ¾ˆ£?°î儆Œ8?™»¯[ß?ÉbAμ?¨ß…Ëze²?î¡´"? g »Ö'?*€£S}Ãâ?CiZ¬'n?¥Ê7JŠ'Ó? b6²cà4FGL J1331.7-0647?ïÿûäE@KY†üÞãPÀ;ÂHåL À<žw{@áqF>RÌ?ü™ƒyœ¤?Ïm"ÝzÅ?ÓW,u©Ð@»
,©¬@6ŒØ–¸¿Ë»±\"?ïø €´ã¿ËÊ+éÔ¿à›¾'1H"¿æW9''¦¹¿á¹
"BËAGNbcuNVSS J133146-064632?îÿûÅnó?®º"€ôÄ?z¤€Š.å	?€
é<¸S?™Wg/•ãº?¬ò48ßí?îV^(í›_?£º¤y1'.?',º&™X?†Ö(IÌ?¦îçóò? yé·B4?ì*8¾ž8	? EÒ%1w?ôʬèp%?‹ÊFƒ‡k?·1_Ô#®?š	›Úë‹?ëaZL? b¦|®KI?ª-2îm?"úü–?·Þ"Ÿ`?™75®ã5ø4FGL J1332.0-0509?ãJhH`8q@Läy'¼VÀ8¯ ÄÀ;'ŒÂÂ#@	"'›Ø@&Ð& û? Áø»ñÚ?Å[ôœî¹@ †/Y‰ß@»û¢£-—¿ÓéŒÁDŽ¿á•"Ì'úò¿ç–ªÁµ£¿êqü!#;C¿èÜ"¤?¿ïÿ±Æ·	AGNfsrq3FGL J1332.0-0508PKS 1329-049?ïjp‡zQ?U-†®?ôùJŠÀ?€Ø3Pþl?ƒnÿӗZ)?†õ]ï2°ú?ï0\µÄ? ¦›Kx±*?dlü˲N?{xNÁ?—`tÔ¥Ñ+?žByW`˹?íÝvXòU? ¹²br¡Õ?› _¹s?'ž'¤0?¤Ÿ
AÛq?š%^èCÚ¶?ï߇Hð}?aJU0;4&?Nn²yGb?E¹
Ù¦ÌÂ?hÝ
qªé?^ã¶KJëä4FGL J1332.2+4722¿í•Ò¢y½@Q篷éÀ:]N[­¥ÀÀ<tZ5Ö{¢@E–hâ˜@Å1Àll:?À±µY¾D?²†¯‡µ#?ïOo^²'å@
$¤¥p;?ï¿àÀŸ—à¿ãiWaæ¤å¿é-h]â^Y¿æ°<g™í¿ëñ§½s¾i¿ïí…èÜÎAGNfsrq3FGL J1331.8+4718B3 1330+476?ïÍp¦Þ|?pÁŒ—{¹?X­ÜåÇO?RÖ| %¬?s5Wƒâ6?m!­–›œV?ïtjQH(Ð?=øq¢ó?Sß;NR%?bIœp?4ÄãFÌ?â2ðjX?ïü'Sۘ?ƒˆBZf?q´D7±5?`yUtl˜?šj
¶ '?1o`9@Â?ïE'J[Þ?{ƒ=ƒêl"?'p#êwc?nÑÚ
†]î?Œ/IŽ±õ?t7ö>ζñ4FGL J1332.6-1256¿ãnjõI÷@HYµà÷üüÀ8ݜþ¨èÀ;.
—~6@†/8§¼G@8"üS£? øÙßɘ?ÀÄEª.<S@ØFèòA@õxèt¿ÕH­ûŸH¿â׌™¿æ=é¿æЖP8ýx¿éL!`ø¾B¿ì
Gahz¾AGNfsrq3FGL J1332.6-1256PMN J1332-1256?ï§à·g?›±Ä"Ù–b?sÔµw¿â?€2âQ­8?"ÎЫ#W?—]›¨¨ó&?îÒy$®-×?¥›3˜n	Å?rÔéø:Ï?ƒˆßXö+n? }Ðv»,?£¤Q[3-?î3Yš]·1?áÙ£M ?—õ—æƒ?'
Or"? ÏšfâÍ^?"UU}>;?î˟'oë?˜­h?"ö̑Ó×?}Q?ʾÏò?ªu'âdm?–WaÛXõ4FGL J1333.0-6626?æl.Šé
ÜÀ9æRlÀ9åüágŽ…À;|Ëëü<ý@<r‰à>@9Eßaô?Б} <5?Òb÷{Ìÿø@3.`e›e@QøV¾R·¿· o Ê$ý?ëñ_ˆ{º¿çGQÞD‰¿è³¾smµæ¿ïÿ틉5ž¿ä9óEAGNbcuAT20G J133254-662826?Ù®·8g?Ãÿ«Â˜‹ý?˜¯ïÑ®òU?§—]D•{?â·)x–ì:?ÄÃ`e û<?àUýJX_'?Èzi^-mö?Žó~Õ´Üí?•l¨°'Úö?Þ\it¡™õ?ÈeŠ -?ڃKë£	i?´9aj«?¸Á¦üÓ(?™Á—mÛ?ßxCªÁÏ?³¬'Io?æŽû Ìo±?©+-8&~?©Š6íQÄæ?"CB=rÙ?Ïa…ÁyÐ?¨¿Z¹‡ðX4FGL J1333.2+2725?ëϾÕ@T,¯¢ðZqÀ9åkÅKÀ<ƒˆ×@yÄqßk`@/${	‹š?³5ëId¢í?­/)ä*—?öôLfàà@
"ÞCÿ ÐU ùè¿ãX˜GŠM¿äH3
‡¶¿äbYDzä¿ç#…uö&b¿æz˜í¢/jAGNfsrq3FGL J1332.8+2723MG2 J133305+2725?ï"ûÏ~
T?j˜oo•?T "°°Æ?K–Âه^æ?Œ?•?õ¼v‡ð…?ábšY?‹LÅ0ý–±?KŠ¶3æ±m?]«w¹›¯?‰ÚÜDþ"?‰»~fˆÕ?ï6pçfð?‹¾Ô'?h«m«i?Rå";
Uì?–(~5q,"?}¬ †œV^?器7'?l>•%Î?u¨ïYê"ò?b['ûƐ?uúôå	È?`ì̚2´ƒ4FGL J1333.7+5056?֛F‡@P7Ù+à‹À9QpXW¯êÀ<&€Aÿ@Ž5deÛ&@oZµ?©Šނ›•?¶ðBrÁ=¢@äLæb @QúÝv?ßÝE€gÄ_¿âïÕ¿ä•`ß鵿äl¥¡·¿éJS
iŽ¿ïüÒf(SAGNfsrq3FGL J1333.7+5057CLASS J1333+5057?ïݏ¢]•Ä?hí²Gà?QkQ?L÷xw?iéPì¢|?dü‹'çâ?ïžÕÆh5?‡à€#¬?HΕåîN?V zÕ¢9^?†½Ðð#?†5ցÊ?îü£üJ!/?"ÒýÙëœ@?~FD¼B?t~ ¢it?˜Ùïu4ëB?ݞ¤Àóº?ïîê:œö?MCã'_ù?EAcÈÎö?6ƒ/Úw‹´?YBŠØá¬7?G"(:ÜåÃ4FGL J1334.1-3521?¸Ú°æl@:´óý">6À;†qž¨ÍÀ<µ—îáË@",Ò£üI?û e›eK´?ÇÜìš"ì?{øVñÜÚ??¸=¾./?üKÛÙ=§¿îGø½Ÿ¤?¬ÜUÖÌ?ïçB.x¹O¿º‰#ªª
/¿ê<Œ¾÷Y?Ï1úcˆænAGNbcuPKS 1331-350?ïwÒú]íë?—Dx
EX?Kó•nø ?ON¿cN?-a–ÊÖ?–¤Mè8Ì\?ï>#(_p¾?–ìË{}7†?\ÕlΏ'7?pN2T~O\?–nD'(ïQ?•³š7ð?íqdE=xŸ?—!ŒþI«ƒ?Š]rtîœ?§,÷$ì?±)/‡vxt?"§@"c‹¬?í±FC
?™&þÐ?y5¨'ÊA—?t¦\µ¥ƒX?°ä#DË:?˜
x	}߄4FGL J1334.5+5634¿ÔŸ/z0@MÈà"'À;J&˜=™À<¾2‰}Ã@ÅSÅ$ù@÷çbzH›?ÃJÕ¦»?¿ b3Ѿ¤?ܦÆ0<‰@£úü5>¿î3(¶ØnÁ?ï®þ`¿¿çêUp
¿ã½¢W®<¿¿êøýâïN?Üá­å+}AGNfsrqTXS 1332+567?î³@S'?ž¨$OÁð?…dluƒã˜?ƒ+nµ§ê?žå¿`Z++?šØ~±ž.?ïn`²Ý]"?¯Ã6%î?Séši'H¨?dŽ½:ôàÆ?õOý¼)?Œï¼ÈIÚy?ìÝ,éçì)?œºÁ'A ?'–
2Ôç0?"	ªËd¼è?´qddà?—î;œRé?ï1Ɉ"Œ?ïÏúõ.?€jöR\p~?q¼e)À±?''SÕív'?|—A‹Gö4FGL J1335.3-2949?ïý9P'Ë@@
=¢ø½ìÀ:_ס<%JÀ<i'Où<—@ÏÄùÛ?ÿ@Íù¦J?º[ˆ'ßf?›'ù†-?átþªëQ@é
<€?î&üX«'À?ÓsºÂ‰'¿âþiȶe¿Òi7;«|Æ¿ån)¾ÀD©¿æ¾[ÏßAGNbll3FGL J1335.4-29491ES 1332-295?ïۆڏYµ?aßTSWæ?D³|žS×?<e¥þ6¬?oLcQ~·=?`?Ìy
O?ï¦mÆ÷OL?…ä#zUq?H4BZè?X/è{Yã?"áN‹˜?"ߔؓ?î¦8>ï¡?ˆÎh´â+h?s3
Šê^0?eTˆ}Ðå?£6_¨£á?†Fn‡ÿ?îåòfžô÷?²n¸-?…½¦ÓÄȆ?pçþŒ.·?˜bßÂ>üë?zbLïÂi4FGL J1336.2+2320¿ä܇ã8Éö@SÌs-õÑÀ;:ØC""À<ºoª²Æ'@½mç94ª?û.ʸöV3?ÓÖBAn	s?ͽ—»!ú?÷إ̭Ã@ۅ9D†?ë·Ç'
0Û¿ì=¥b$¸F¿ÍºÞæ¿Ç°j–vÏj¿ç€…@dž¿ïÿÀªšëAGNbll2MASS J13361219+2319581?ïí†:J?£""1z€v?f
Ì4ɟ•?'òÍG‹F?›A¨Ÿ'˜?¡hK1
*i?ïg8l¹÷?•[øa?T)çG·…·?c‡zÆ\(o?'ÖQ]íHÈ?"œ³>?íÙâL
9¯?–[ÆÀYd?{'û¢Þv?pòšƒËe‹?®ï·ÿ¸	3?"Ü9±@æÍ?îzW½õ½	?‹Ý°ÈfŽÑ?tf˜Ó]ÑB?e'æ‡S›?¥Í±8uM?‹CÍ|Ç1e4FGL J1336.2+2053¿æ"¼ÝìYÛ@SÿëJÀ:ã
æãÏHÀ<•¬Þð¼@¢3k½=c?þԓj«p?ÍÙ_m=p?´".›säS?ê–
ΐl@,.Œ…_?ﺌޠ3è¿äÜÃàj
¿á‡—¾V迼e®Ûu1/¿áƒ"Ê/c›¿ç×_f˜AGNbcuNVSS J133612+205102?ïk\eë?"ihÐ_ð×?Bˆ—Øõ=R?5"¤–ò
>?'/Á˜®?"Òö*ãÂ?ŸÙè?‡x¡àõL?E"1ÜzRR?U¬÷º<mr?ˆ¼Të÷`?†€ŒÃw<?î£$׶?'öq7aa¿?r©þa Ï—?\Îô|pÿw?­`æOºª?ôÞ"º)?î¯$G½?ˆ¹N ŽŸ¸?p™~ñÁ/?_nŒQàS¹?£
ڇL	?‡°éöÚw<4FGL J1337.4+5502¿êo<dùîˆ@Nm©CZÈ£À:ôå‹àssÀ<¤ÝŸ'ç¦@_o̵@Æ"ï¾?ÃãŽe?•g³™ú"?Ñrd`ý›Í@
Íî¿›\¡õ*0¿æp@o[Øn¿î8¯6Y¿ÍÈ#à{Ö¿àAœbKό¿ïí…>˜ÂAGNfsrqS4 1335+55?ïèçÓ}O?r>NX@¾?Gkñö,?C7Ô7qÙê?a=æ®þ¥î?qÑéb|Ç?ï¬*j‡ê7?ˆ
9""?Aaç(>Á?Y'"VQ¬á?ƒßF끐ß?†Ú9çñ'¡?î|…—ÀÌü?—²qB=p´?i©³è÷Àh?c5ëa7?¦Ec´-?—X¸(Ì?ïâÎUIxU?Yº`ÅQë?H­Íʇì?B–‡Uº|?g?Ch?Vk¾ûE¦/4FGL J1337.5-7802¿éQÉ5`"À.ÉÄüó0À:¾eò£ +À<jGW­eÿ@l/µÐ1@¬¸?wT?ÈÍvÀіá?¸]/ÛåÄ?ñtVéò?é&ƒZ?î48Ùeb¿éÄ×5›J¿å"åÕ²O¿ÐÓDá"é¿æŽBM'j¿ïÿ«Ÿ7=AGNbcuRX J1338.2-7801?ï\­þJ9—?ÔÞC¾ƒ{?Qý#[BJb?OqXœuL×?"Jn¨¦?,^TY#W?êÂÍn'@?ŇíA¶*?¢Q|#B?®°±²–Ý?À`l­€9©?¾æ¢K{?í‰åDUr²?"¿
ˆ÷e?~õü>b™$?uê)RµÁ±?±Ávn@Û?'ÒI›a?Þ_¼Wr?°!Â)Ã?ºÇ´œ¶Îi?¤<ï
Ùª?ÚîVÂ{4ó?°¤I"ì"ò4FGL J1337.6-1257?íj'ê2kì@H0W\gÓÀ8¼^ÑF¯À; *o?Rü@€|»@p…ÔÀ·?ªâ¹âÔú?Á·œäÒ¨@÷x‰|ì@;ñ®ƒ‹?ì赖Ob>¿ßI¼±K½¿åºß.Ï d¿æÉë	ζ¿çüQ¿æ4}¿ëãú !°AGNfsrq3FGL J1337.6-1257PKS 1335-127?ï™HÄh½?ˆ†ƒäþ¼Ñ?aäŽÎæ‹?`M¯ø>¾K?…4ۍ2a?†©ª±¡­?î°ÌË_Žï?žSyôÑM?w£öqî…â?h7k4|l?¡þ´{É@R?™Â+Ø­÷?îÓé~'Z?'λ|§òÒ?}ÆUøî…?x+¬|rX¼?ž:¯ÐÃÚ?úŠ\üD?îL
ZhV?Ž×oLìx?–ñó—6+'?ƒbäÒõ–‰?£RE^¾dç?‡R‹-»o4FGL J1337.9-1956¿î}¿®2E@DÌsWæpãÀ:ó/p0ÄÀ<;+äŠX´@Œ·ÔCé@¶5¾þ­ð?̇À键£?¢(^Etm?ÕØÙJ‰'@
lš­•Ïà?튌Jü}•¿é¨USïk]¿çN'ÿú ÿÝEâb`Gh¿åšVÞ3&ž¿ðAGNbcuPMN J1337-1958?ïê)¢"Œ?[$Vv°bÅ?7G©&ë?-P‹ å"£?bíhV¡Ý?YO?_?ïhãÜnH'?"^¥·åg?OqˆII	Ý?abwì©èã?'çø/ì¥q?'{LïXÙÌ?îuB¶¾?§D·Ù?qôè²kÍ>?eS<Þ¶}H?¦m7‰†žu?hµ¡F&?îÒt'È¿?"RŒÆu/e?\l £wÁ?J
,(:L?¡õUÞbö?"	´$"Ñû4FGL J1338.0+6534¿ã"…;	@In¤"‰—ÄÀ:d¸ÄL0À<…Ö9ïæ@´`àÀu@!‹…ÚŸô?ã%Éé±?¿6Ü
,~¹?øôèû¼¾@
)Öð? °XÍÌ|¿æY	áÖZ¿æºl­¨DW¿ê"öÕ®¿ïÿµÝœþ©¿ïÿ‹Á>ÏAGNfsrq3FGL J1338.9+653287GB 133543.8+654752?ïçsûAñ?bPTÿgÊ?OƒI46Z?K	k‹t|?`«£ì¦;?\ïj<Œæ?îäÅ·¯?›«Ü-• ?jÒ~¸ž)°?uRËág2? |£"Bf?™N÷Ô|›ñ?ïBæ'gº?'\‰Pg'?qùÒîÔl?^>#y!6 ?›9.'S¤?€omuà[K?îÀ¢+€Oü?"µY	S?"Ø
C?z²2f'Fõ?"äâ…当?~ÊjG¤4FGL J1338.9+1153¿àô#P<-ƒ@QÈ\|ؙÀ:»WYƒ)À<XEq
‰@òv`¯m@@uá;ÚÂ?³AwïzÌ¥¿–gڄÆMØ?䆼²£UÛ@ûû!ÉÔJ¿æÁáìï'¿Òƒ`½Z¿æy¶Vi¿Ýá‹5RÈ$¿Î†Ï'y꨿è'?
äAGNbll3FGL J1339.0+1153SDSS J133859.05+115316.7?ïݬ?‰À?fp‹ãÐ3?9ñìÕ¹ß??/™YÌ'ñ?o«%¿Ž?ea=•j@-?ï¸C¦
‡?ƒUw¦w]?92ôx|6C?Hô7c?%¦ò¹|¦?'·'Ç"?ï#&Ðr?'—¬19?eorn*{?`ÿdž5ò+?š
§Ž¸,q?-Rþ3?ï·`d²
Ö?f&ÚGÆ-?K.|ýRè ?=w1¨§ú1?€tÿ¨Ð?e]ŒZN­ï4FGL J1339.0-2400¿ê–NÃT@BËw[0À9përáÀ</;©#z@ÐÃ7LÈ[@÷3¨£ù?°k̬Ái—?®ý&¾%.?ýt,!Æú%@tn}·÷?äuÞÿT^¿âJiæM§S¿ãqø -à¿ãô±œ]™¿è~¶ôô3C¿çR¾éµ;AGNbcu3FGL J1338.6-2403PKS 1336-237?ï:¤+ia?'{ÍÅD]u?_¹éIO"‰?SÕí5`åq?–ÁÌåýÛ|?'äŒ?aWû?¿Ó +?…øi®ãÀB?L±­¤½³?`à
].?‰'µ0ì$æ?ƒÿfÊ%D?ï¡m
d_?mpúÛò^?o ,Ë;?ZÑìÕP@û?™7ÌÄì™?–wùj?ï{†c®ÝÕ?rlýÄ_9ç?s6"Kåü?[åï4n¢?‡ƒ$îUŒÍ?m¡ƒî³Ø°4FGL J1339.1-2620¿Õ'ƹå@A¨hۋ¬qÀ:u\€3—À<o'OÐ!ì@_y';|-@RÑ84$?€*ä ©?¹LuN‹©A?öÈÝ•.@
'áG®{?ïJùùUÁÓ¿å½K_¤Ö9¿ápXô©¿âÙs8ÜÀ`¿äÅ"}c¿æŠD'HAGNfsrqPKS 1336-260?Æ=-?|ӗ£ÙoÈ?IÀ}sªB¶?<!i)ž"?†Ÿ·6{?|¹>‹¨Å?ï X?õŸ¸?'§ºvÐaI?A¸^Âtµ'?PNÀ€âç?†ÎjpƊ?¯½eqšÎ?ïÿ×@®Ÿ?ƒGÇxi¶?l•Û€¿q?Yj\|Š€²?œ-I¶I?­Þp;È?ïYì
ä
?s"tš#j?côµÔ.#I?J7ÌVÕÐä?'Cçèözc?r³½Êµ4FGL J1339.9-0138?ïF\Np·‰@Mzj~ùÛ#À;=[XkÀ<ÜãèrDÁ@‹‹ØeÝ@ñ·D¥?їÆÆ"Ž ?åÀGƒLP;@Qͽ"©@ ß=è˜Û?ïõêgèF¦?ÜWžbP2¿âG~>œ¿å @LÜ'¿ïÿ¶>@£?ë\e[¤k…AGNfsrq3FGL J1339.8-0133PKS 1337-013?íÝwZ8?°j­o,?§¹ Ó£N?«¿xÁ-pñ?"ÝÓ'`ý?–OeÍ?êêpÊç§	?ÂÄS'Ž÷t?³~}cèF?»KaåF?µ-üŒ^ßt?±Ämzrö?äÉrg¿ð?²ŸðƒCáo?ËòWë$ô?±¹úâòÀ?ÀçßM›K?¢±ñÍ»r?ì.–àIß<?¦¤I˜æû?µUëB e?£ªŸ/?¢j»w!
n?»&ïXy"4FGL J1340.0-1501?íaA¯*ƒ@G›¥ãSøÀ;XB 6mÀ<®Ö0ù@!j¼<ܪ:?Ûeºnü7?àcÞÌ©'^?îȐB@™½ÆŸŒ"@qëô…M‡¿îôŽŠïˆ?ïñ4?ø"z¿êì>ý–Ä'?²Ë;A
€5¿Ñ΂#Ü(4¿èMnGÜ7¤AGNbcuNVSS J134005-150314?î_‹ ?«O7D£B?Š^"±ËJ¬?Œ"0µ™ëO?£o­9ò?§ñ°¾b}?îÂè¾Æ?¯ðèb&Û?€CŽÈk†æ?œÛOºZÿ
?Ÿ7#ñxå?¥Æ	F=v·?ìŸtÂk?¡Gb'´?'TM(Â	?€K4ÐSEw?¶¯F¢¡u?ŸF}_1`?ì‡Âz¶a[?¯ËäqI®)?jCz'Þº`?uÄ4
Ó ?ºïÐY
ÿN?°LKÿ ô4FGL J1340.1+3857¿ëûîJ 
@R™çW"À;3
s†
À<°¦°ÙQ@@§;N
@>Ü~ñw§?ÌӒy>Û2?Áîj@æz?îuà÷üü@@躹¤Ò?ïÿȂeJˆ¿ä­v€d¿ë]Ä×5¿à °)¿é•ã+³ã¿ïßÓo~=AGNbcuNVSS J133849+385111?ïÉEA¯q?z5£Éñ64?aƄÐÊî?jÖ¤åX?rz¿Ò¹"?sM€m&?ïQÞÅÜ?"´àB*‡ð?ZžÝ´¨ø?ivüj÷ñ…?"#Íob9Ý?'Ay£ÆiL?îZóáå?'6HôõÍé?týCæµFÊ?l­è—'dá?§¾˜EHÈ?.%ù—N?ïhWeÊÙ?xL7ƒ'ò?zn{8´fÅ?inÏU'?ˆ²þŠ3£?r,ïj"˜Ý4FGL J1340.4+6926¿íR̸k8@GŠpCßÀ;µ?ÇÀ<DZ«ß{@dlƒ¶ÙF@v†a®pÁ?̎	Ãx:N?ÂþgN˜¿?òMº°k@À"CÆÿ-?ïÚKäÚá¿jÓaL²Fu¿ë:ñ£EêÆ¿ÙÛˆü¿ïÿÿÊPË?ï½%?T©¦AGNbcuTXS 1339+696?ìPZðPô?̝Á͊$?˜-ØM?²~<;Äæ(?·u¤ré/?ÆâÄô/0?"SD?"ÀËá"-?Dû@²›š?_ÍZä?ï?‰;wü?"É·º?î"C5^áo?"ÍZ½	c?€´;3HŸ?uÌF÷´[?©®½ä…æ?"RT¸¬?ïôvh‹}?F7yÔÄ?+ÝvZÀ? Ò(D…»}?S—Œ::›Œ?DÌN3?¥s4FGL J1340.5+4409¿Æ¤vAzÊ@Q"¦ YŸÀ;•/§xÀ<©u¹À€Ž@"!ä*7?ù¶È™aev?Åʨ…DÎ?¬°Ä¿žLB?åš>o§WÈ@ùŸM㍮¿èìðùÒ¿U¿ï"8Á½z?Ü5-vÇ¿ÏöÈlàÿ¿Ø:ÀðÒ¿£-oàô³,AGNbll3FGL J1340.6+4412RX J1340.4+4410?ïa¶…?
HLåÛ?B7Dv³?88œ'Üç?"0p"'è?Ž³Ž6æs?ïI§­Èè?¤Ô ݯ)Ð?M@Œ]õ p?`s"'¬ó?•òf§W6)?¤‰™—h:?íô8
"?'¬¥ri?j¿(¾?U~Òu•
‰?¯üÒõO?'AÙ;ôhz?î=ËbÀï?"Gþ>ðz?[fhñC~?Rg=?«S€Iؚ?dõ¦.zð4FGL J1340.8-0409?àO5ó,@LA]€ä–îÀ:Tò÷ÙÀÑÀ<^=ç™@µ|I| º?þ®³Ý¾?ÂÓë9Ÿ]ÿ?˯D%ɾ%@
jOv@'g…d¿ïԖZIør?ïÿþBe«+¿Ùì ºŠªé¿áÒ°;œŽA¿å®úS¿ïúX¡+ß,AGNbll3FGL J1340.6-0408NVSS J134042-041006?kÁ`8?\uԛL?yÛhuæž>?råN¢J¯î?€,°Ô´¢¶?w'Üï¼?îëùªÒl@?Ÿ0s!u¤"?vaëü˜OB?ƒˆښr`?œèO¦Œd1?˜Ž\'·x?ìáM%Z€¹?žo"eºý?šÇöU,ôg?>àe‹G?²C™?à½?"'s¹³?ìmF÷ýW¨?–¼'.éC?¦Õ¼ˆ»ˆ?ŽºánHzg?±*éû·´u?'W‰{b¶4FGL J1341.1+7433?ä†??#€@EI¾ó(À;õÙ7>Z¯À=8XÍ@!m¡™?ý>½c£>?ξ¿ƒc!b?±í{˜ý'g?èÙ᝿C!@Wê°¢¦¿ð?ïÿùJYQ¿ß ªº©3À¿ÝmS?˜j¿é"Î^G^
?à…ª.<SmAGNbcuWN B1340.4+7450?ïªé=µÏd?++c§?Du˜2 ÁV?B™–C"©×?ƒþWj?ŒêQàr½?ï™TU©2?‹K:²é?@ l•÷?PÁ¥^Ι¬?ˆ·ä!E#¹?Š"*¯ö$?íñß¡p?•fý¾o4ß?'Rr}çÍ?'AH  6?¬Msªß?'Š°éˆÈ2?ï˜(¤•€›?w¬-8l?a'÷ÉûlE?W…¡tJm?…'Xè þŸ?v¦«µÆ4FGL J1341.2+3958?èח˜•k@RaÞ¨—cÀ:´4'D¤À<ÐÚx†ú@ ›Ó¾®{ÿ?þUÃKCË1?¿£«@`¿";$wj¬?Ö¢WBÜôb@üP#ÙÎé?ïúÖ*C i¿à*·ß)ñ–¿è?¯Èe_¿¹¸þæ$¿×ú3ÂûڿގH,¿{«AGNbll3FGL J1341.0+3955SDSS J134105.10+395945.4?ï•uzdÛ?‹¤»'‒?W_±m®gÚ?Pàb$Œ?‡¶«9ro?ŠÓùü2ß?ïœ`Æ¿,h?‰",;}œ?EµÙŒŽÆ?S(	D1Üú?‡Œp·lY?‡è¯Wéª?íÍÛ{à??•@Ñ8S?ußô6zV?a Ÿøú?°3$ݜP?"Â󬇜Ï?î¤W=?¤£?ˆUáå2ÊX?ƒHW.rS?tÄ¿ÛT"? èv`i3È?…Ëbövbl4FGL J1341.6+5515¿‡ž·KíOŠ@N7°ËæÀ;«GhGÀ=Í 1cO@˟P<ÙO?ÿ0–‰B?Õ6]ŠÒ?ÄAꛔÆv?ðÖN™@°	j¿ïÿ3Qf$!?ïþ5$¤ú÷¿ÉŸF—> ¿ÝFéÞÖd¦¿ì.U'ÙŒ?¸Y:®Ò'AGNbll3FGL J1341.5+5517SBS 1339+554?î†]£ä±?«"?0?{q˜UdÓª?tÒxK…*?¤0çˆ?ª:ª»¹¼_?ïC0xP?–ÿ&‡Ó–?WŠ$<"?fóL#[‹?–!]m&¥|?•`îÒýð}?ì¼Þ3<¶¼?qÓ'Ïï7?•ç¸‡ØïÐ?ˆô?¥`¾?´Ÿ D$2?˜ü
›ë"?ï/ùô_}?3'2¹m[?vxƒéG8?i"eo0,?"|Á@y¾?~œÃBˆÚÃ4FGL J1341.7-3907?èìr$hGÆ@6·Žâ†ruÀ;›¡Ÿ!˜×À<Á_s-F@!ë¹½ûN?øŸåÉä?ÖFlÊS?Ĝ:HPPÐ?ên±XÒÿí@AP5ÍlZ?ïâkªÛ
¿äòõÒ-_¿ïôo"͊?ï­œ®÷пë‡ùÞþ¨'?ß¾F!L€âAGNbcuPMN J1341-3906?î£Sÿ"%É? âb'Ÿ];?nK†–…¼?j§A˜¼R?£æ¦$;$? cM'´õ?ïZcÂÁ?™wí(?X®AzC×?q¬Ð‡?#Î?"(»ß€½?—Ç泃\°?ì¿%t/õY?œ#+Ax?†hVi—n?~|'ö2 o?·9ɑMgl?š8V‡n?îÇêoLÆ?™íñ&2n?hOc‰òåƒ?rëýÞ?¡übÕ|P?™7±ˆÿ4FGL J1341.8-2053¿Ùæ™&­@D:[–(ËÑÀ9ÊàÆ~ÔòÀ<†Ñ?ù@ÿ¶YÃÀµ@t"« «?¼~)¦—ƒë?½[K?Äf!?ú4§Ý);c@®ã‡¤z¿ÝF—"Ûâ¿äñiϧr ¿èÂSAp²¿êªüóF¿éØêýºU|¿ðAGNfsrq3FGL J1341.9-2053PKS B1339-206?ïó›gØNÚ?t8=ì«H˜?=Æ¢!?[º0Ml?QW«¦âHk?k)¡Ÿe³?l?á÷wR?CN(vâÕ?S…}¥O¼g?ŒIÖrp<N?œåô33?ït›È?ƒ¶™]hz?sý*Yˆ?pR¿Hõ ?˜2'"#é‡?€ü°n
òs?ïË3·¢x?a½ö(ÈBŒ?S\4 ±#=?@Uu†¤?ubü{Ï?`AsfrñW4FGL J1342.6+0944?äé']ÿÔ@Q4Z_Çæ´À:||ûÀ<€"ï5­a@¬ƒV6C@‹°'ݾ?Â77º+Šr?¶ÎùwМ?õL{ÃŽ@ª²W*´4?î°ßóE2¿Ó֑ýCD¿àéâoܿߥk*±¿ç2F8Éu)¿æ–øÕiSAGNfsrq3FGL J1342.7+0945NVSS J134240+094752?ïa¬Š2?"îpÞ«7Ñ?]	y¬\c™?PÆÁPéDX?'ù×3?"!õ¯_Cñ?ï‰ÑxÑ?Š	6â7?R¨J•O$?`¦Úžîd?‹6˜¬jê?‡ã÷î'>?îËîù¬²?…&Ðno½?qº8%B†?bà¯8ò¼Z?¡	É`–"'?ƒ"a»ýÜ?ìV?ƒÑk¥†&?Ž_\-Ò?s#Ñ/қl?žƒ¯·Ü^)?óÌ	c<4FGL J1342.7+0505?ÖÂ-ê
Ë@P3 ٔ[lÀ:…̹–nÀ<z
Á$"@´¥§nïL@lFD‡ïM?¼èÁÊæÌ¿`àéè?rï‹y×m¡?ÿÓhõâŲ¿Â´†…ß¿ßíÞҞ¿çpLÎå«Á¿ãAãÀe»¿ëp8à?á¶?Á8AGNbll4C +05.57?íë¨.RY?¬ên3êÂ?ˆw`çKÙ¦?»Ç!òê›?´y¶¡£ò?ªFËi·Xa?ï	Ø8œ"?šŒ³=‹Ž%?dUN-lx<?qxFr&¸?œ:O&Îì›?˜{¿¨o¯?ìя]yõ ?œOé‡Ä¸_?–§Í˜	w5?‡ÊõJ»›?³É'®-õ"?•'SRVòß?îŠé¤Œ±?ˆ.–Éæ*?I`'ŠW§?wœTøëɕ?Ÿþ-9Þ?ím"†šÑ4FGL J1343.6+5755¿ïò{½w@LïQ½aõ¾À;CP8&·ûÀ<ÃÕ×7‰Ú@½ÃIâ¢@ÊOv`?Æï8&&Z¿"-"®jƒy?½*¸TÌ`@ëÓSú~?ïÞ>y¸R¿ë³â…›µÔ¿ä™V³jû÷¿é©YàÆÿ®¿â7EçjÞ¿ïú°€²AGNfsrq3FGL J1343.6+57536C B134209.5+581020?ïåõ, I?nÿñv²Þ<?=)ÂÁ¬—‰?6±j+û¶'?f—{*#Œ?m‡¢ét\?ïI›¢w*î?˜þç‹MR?Uº&Øv(µ?eõ™›ÆQ?•péC"?»?–çIäÿ'ä?îJ`¸£ªå?'ÃL°ýã?pUzër¦?cæT"éQA?©OE5gãe?'+8øQå3?ï¤MjÃé¢?pÙÀmëbæ?_ćYËiÓ?UILï"U»?'ôcÌ*F?mù¨|Lƒ4FGL J1344.0+6605?Ž©Em¤F'@I™" äÀ:›wTË3pÀ<«"¶
+@–6ükuð@äìé¢Æi?¿8Ȑ‰¦?°£€ùÊ?íºÞEÆ@|™ÒÏp@¿á¹€¦ƒ¿â³Eqú_¿ççb\«¿æ¢ ©XS~¿â¦t©H›¿ãŸsbÎ+rAGNfsrqGC 1342+663?ï{:»j¬«?"òÙç×ðv?^§ÿ ?M"Ìþॏ?m¼%spç?"9²ŒAb?%F?ˆbÛJáC/?K8í>jÄ?Y¹ðsµdù?b,ç‡ê?‡-¸"—u?ï=»)?e
Ïg?iänB}¡$?[ý­mÄß:?™ÛºÖ®"?€yd!?ïâM;ò·?s|dײ¥•?o`ºïàø?Z§ŒjôUp?ˆ/=õÙá?r­¹Ö®3'4FGL J1344.1-7700¿ÕgiÖÀ,è鳍aÀ:j{Ö:3ØÀ<_ÐJ/Ï@dá59°@ðÏü,5é?ÇߋÁ>Ï?Æ˦‡ÙL?ùÂ=ý'·?õÂ/)ä*¿ïïwÀOç?ïþõU9¿æRÝ^ˆ¿í©·ôÎs–¿k*ýžj¨"¿èk¦âWxAGNbcuPMN J1343-7658?ì¨/¾³r?µÔõ>4?—ø—‹
M ?£—.äbP§?´Á ŸGÑ/?²û5P´ß?í0¬ZÂÞ·?³N·,Gcp?'36u«K?š®žð	&u?±ùP\KŸv?¯àHÇgK?ê&3ü'Dg?¦Â†FԘ5?£4û=°"Q?'"Ú¯nš?™ñ?öɏ?¢'bňd?én| cl¬?«M¶×z¸0?¢ª›«X@_?š…ueǹ?śh"œ=;?¨ÍÙM£4ÿ4FGL J1344.2-1723?ïýÞ¨v¬@EÕ¡"úÖËÀ8ðÍ¬üÀ;Õàl¼Á½@.÷"ûR@ÙªæÈ÷U?ª´vØz?¿-¯e³¹@ORáNd@ãؖÚw…?Û´;ÿµ'¿Ùs8œS³0¿ã'Í¥&Á¿áš¤'D`'¿æÄì=ÖOX¿ðAGNfsrq3FGL J1344.2-1724PMN J1344-1723?ïï/{Å6z?XCzÄ°ò?G…±Wq?FáÅ
ôæ?VEœçRû?QœNçµ¸?ï~™Jeå?Œ@i-v?NnG«×?`Â6s±¿‹?ŠÀ7¶'7?Šn÷ìó]F?î³Ïì³?•dKwüM?‹YӔ('ì?‡T»žW?›ÙŸ‹¼½?9€aF£&?ïäuf´?X足}5?Aqà0Ö?3 ®–h0¬?g.!í¦?Vˆíàæ4FGL J1344.4-3656?í-ž/Êå@8¼%á;ÛÀ:6,PÀâ´À<G‹³ýÉ@Y/'éA@£Cœ7Ì?¸Ñæg'¬l¿tª÷ºâ?ã_v¼Ï)@:î¿»Â8¿ÚËÅ:Ý ­¿äpŸ¥LU¿ä´àFý¿å=µ¢ä›ö¿âŸÐJ/Îû¿Ô‰þ¼3!•AGNbcu3FGL J1344.5-3655PKS 1341-366?î¾Ik*H¯?"P
³f?4¼é‰Þ?qÅP'fÇ? 4æµ¾CÈ?'þòÀc9‰?ïCÓz)\¶?'ÉÑǥѰ?YLR Ð;À?cܟØà#?•ðːÇe—?'£ù§tí"?íò¬mÚ¹?—ËY''?ŽçQdQÙ?zÈùÍîÞ	?³{ˆ²d ?"Ö»aT¨?îOƒê±?‰îª;C6À?"ীÞ?qP,"Ÿ#h?¥Ïͬµ$º?‡ì‹ºža4FGL J1345.5+4453?åQ ±Ü1@QM#c²WÀ7&Š
4›éÀ;q%SvŸš@|Bµ²)@^á77¥?‹›ó]|ªB?³øf>ßu@&y•în@ »ˆb¾¿À
lÐó.¿à Êƒ+¿ä²+@ "¿äk¾§›¿èÚ^Poˆ¿ìܞÁ̓—AGNfsrq3FGL J1345.6+4453B3 1343+451?ï†Ð¦¢EÞ?"6{?`Wœéâ±¾?`<!SzÛ?Š5ïõÜz?'{ø9¢Ý?îìk?£¢¿ªÈê?yߍ"ï!î?€ñ'[x?›êZ'êU? «¯!l™Z?ï8ß-u%?‰áÏ.ߤ?",$eK/?'‹ÔÓÀ?œ=kš?€Ò%•mŸ?ïìÆ÷
¿}?[%B`Ç?KWãl]?IY#Ø}¾?XƁòÊÖ=?Sç¦ÈG¨ø4FGL J1345.6-3356?ÀºXO'&@;—BöÖÀ9ýžóu®À<PS@ôÄ@¾wÎm¶½@W]K4²?µž—°5gk?"?\6a»Ý?Ѷ»"i@+(wÃ[?ï÷À@win¿ääž_Ñ÷¯¿àýXsHͿ㣮¡£S¿Õú7¿	Ò¿áž$˜¼AGNbll3FGL J1345.9-3357NVSS J134543-335643?ïÌ4ˆÿb?sҚ)Á?Bhbu5žÔ?<Aa	Ï ?w˜¯1К!?qîr‹§ ?ïËÆ>Ì!ô?}"Ά+˜?.ôYÑíÙ?Brºþ¶"î?y%=Ñv?|¦ñ¦ú­?îꏦelA?…׆ùTW?i5á0#(?]›6$¡.?Ÿ‡OLsX?"õ]Ѩ?ïÕØsÈû½?\?h|õœ?4)Ýöš$g?#ð¸ùþÕ?sÑ(<~â?[·kNK˜a4FGL J1345.8+0706?ßS–Æ疹@P‹6¤û©À9lì®êc·À<7T+Ñ?"@‰gWË@P†å?¯6lx¤,?ªíŽ
t]?÷@ô@g)™¬c÷¿ÐB~ª¿ãWZYé¿åÎU-XþŸ¿çí`Á
ø¿è¯>;¤ò¿áìÈ×'šAGNfsrq3FGL J1345.8+0704TXS 1343+073?ïÊÂ|™ý­?|%€v²ÂE?Fœ™=|V??U¼K1§?wË.‹^ú?{ÿ‰!Š?ï­á¾QAÓ?"Gÿ;1\]?<ÇW<,½™?O#¸"þ¨?ƒ¡U±Î%µ?ƒNé+ß<?ï)á¾v4q?ï¹Á×»?jýüñ'ÉH?]—ƒ9ÖA?—d"¸?€Y{î~?ïõ	y"u?C@cøo»?6Bs¦ƒ¾Ž?&6¡ޅ?P]6$)ˆ?@ÖS/u;è4FGL J1346.3-6026¿ÊëÏÒ1?ûL'à°«À8q¡ueÀ:¡6¢S|@''•>@-@˜ÿ%­B?°üñ>~–?»B	å²@
ßËâ˜?þªFJ?ïÿÿ" 5•¿Û[gð$–¿ä¶0íÖ¿äù'c€¿èQ
I/û¿éÊßâ©-AGNrdg3FGL J1346.6-6027Cen B?ª#2Êæ9%? Æò
t:q? º
н?áËޗø?í]2¤?©¾U‰
¡?«þ†Ó‡ãn?©þÃ(¤I:?Ǔ¤ósÙ?Âk{`?è[P©Š¤Ò?ÂãxÕ°?ƏÌkse6?¨¯ãðVbf?º;#^m(‡?Ÿè;ÔLÚ?ç¨yU¡?ªâj±Š«?¬;ð¬™97?':ŸRS,F?À…óšäQ´?£É›"ÿ·?êÄ}X?ªêrý£ž4FGL J1347.1-2959¿ï̏»z@?[4ø/Q&À9ûŸÓo~=À<BÙÊQm@æÀ3â/µ?ý"ZÖk®?ºbg÷¶?»à€&(@t G2Ä?þØépq'?散ª?Y?Üg¬Óª7¿ÜxÏ>ìúÀ¿ØÍËz¿åºçÇúÖ¿×`óà·æ6AGNbll3FGL J1346.9-2958NVSS J134706-295840?îÓõFc {?'JÙ)´Ý?z á.–âô?p|×—N?žùçö7Ä?'‡KQp´?ìòöã‡Å?´Ö·HxêÜ?¥¹o˜;gù?ªr¨ÎÐÈ?´ó°|Æ
ß?¨ªŒ6^p?í-žÉÊÄ?˜·íìnÌ?ŠÏ¤3Ð?yµûOÒ¾m?³=õ+/ä?•ˆ4áý"á?åá.4h?¤²ÞÚú²Ò?¿‡ÐÞûš?›ÈlNÊEÀ?ȸ7ɤ"?¡,td¢"ê4FGL J1347.4+7309¿Ùˆä•–TÁ@E¯BöÖÀ:øˆҜÀ<ʔøJ)@‰ðP4¡@)}Ý{pº?Å·?ªô²S.?âÍ,n@/†—3bÙ?ï)Œ‹"Y¿å|'€Æcý¿ëϒ_µ¿á¥Ù]ÔÇm¿ïÿü¿ÙŸC?Þ{©Y*=ÁAGNbcuNVSS J134734+731812?ïêmꇫ¤?cžÛ"ï0þ?^®¾Nƒ!?a=IΒG›?Jød´n©?JÌÑ&ľÄ?ï5]î;?¯)8ÀAp?^!—~a‹?py¯Q†‹?›÷FÚÊRy?®à™è2?î¥a'Ї?d¬‰"ä?vR5é1,?ofI~¤ý?¢äs)¼Ò?‹d×]7'u?ï½½èÁîù?kg͵?lÐ[Æ&â?`vôéú?r¸Ý»õ€¶?`ÞKIÃb|4FGL J1347.6-3751?äôdjÛ£@7¯ŽŸj"óÀ:‡©­
À<ô¬å§@æ#·ë_@[r>á½?º™+"î?É)I¥e·@
£ @¿ä@™!ç±T¡¿€¿^Ð	A?Þë®9cÎÜ¿äßâSFÏ¿äÓsëUN¿êqZ€a¿ïÿl&™Ç½AGNfsrq3FGL J1347.6-3754PMN J1347-3750?î–ûõÖ/??›ŽË'<ê?˜»ËNbÇ?'U\7†e?"dµ÷.µH?Œoˆ¾ûÄk?ï"F´›?Šf|"Ç|˜?WÑ®«ÃŠ?dŽß–<&?Œ¦}a?‡ÇË#B?ìæS,Óê?¡†AҋQù?£ÏãE¤+A?•~Φ´Ó?­È'‡Ž–?"Š+'Ú?îêþu@z?€+§LØÉ?"I³Ý¹ ?o"¯ÕÀö?˜{WmԔ?yq°"vN>4FGL J1348.9+0756¿½GÊ)@Pì¿±[WÀ;'/Lô¥YÀ<ŸÀ_@˜@ 6Í.Çhµ@cpÍÈuO?Äái§c†¸?{ó¦‰?¸Å›€#¦Î@°Î‰»U+?ï!
÷9ˆ¿äi;,ü¸M¿Ü4…ãÚ/Œ¿êq¦ é4¿¼am¿\]	¿Á§Â盰AGNbll1RXS J134853.8+075704?Oý?3½g?Vð†Þ¯§ô?Pº#m÷`e?£`fÉ9¢u?œ l
©(Â?îéG1fË?£Öëç	?cúJ¹€ø?tĸåÚ{k? :¿=ûF?¡¢þvŽ	Î?휕´1b¦?"±88L(?z½o½µÕ?nžŽv˜â¨?±o{b£u?"lŠœkˆ,?îmYOÓލ?'ÆåVÇå‹?aÝ«ÅF
?\¼ÊŽÎ6?¨™HÂß?' çpC<4FGL J1349.5-7153?íUžìPÀ#¾è»¶À:^qS)rÀÀ;æ"4­†¶@:û³•V@Çc»';?»œ
7;€Š¿³ivRˆŽ?û
6 ¥ý?é8.¿å˚gõ²Ÿ¿áu³Á
&¿ìã4–~\¿×çâT1¿á½'á>sÙ¿ÖFÁ#>AGNbcu3FGL J1348.5-71502MASS J13490974-7152510?ã:~X5}®?É×oã»í?"Í_'{M?'TšÀú|ë?ØN-WmSÀ?É£™ñ6Wò?àáIá³Ù
?Ï1Þ" ½?•¹"QÇ À?£Sja¢˜­?ÜáÓ÷{ÓÜ?Έ‹Ý{	û?åüÓðc?²™îå۟š?›ÎÊ.(1?ƒßmGÞ6[?ÒIk~
WM?±ùZž‹±³?â 5FA"1?¶Õք		?¬ÓQ…
Ú¥? ÚxJµ™?×%+BÜI?¶E¸g—ç4FGL J1349.5-1131¿Ñóxˆ'u@HnR'ƒÓ_À9Ñ×ΈÀ<Ñqw;¡@gŽiâF@køüÖÔ?±`'?º×ù%Æ83@1ù⯍!@¿¨ƒÂAÙ¿Ùò½'È¿âYLV¿æ¡*òòÑC¿èò™°?ÎL¿éÓÔޔ‡¿ðAGNfsrq3FGL J1349.6-1133PKS 1346-112?ïæb½ïç?lt•£s??jÑ¢.­A?7†P¦_A)?e¯è;ÊCM?kSXL_?ï›%ñ7Š?‰LâaÕ(?Eg{‰OÚ?X"?ÄXÆË?‡ç¾Ë¹ˆP?ˆ1¼T(´·?ï'ˆÛ±¿?"' ¤L/S?siê¥Kü†?eŠú=|t4?š ";6Èü?'ïg€+Žb?ïó³S¶ˆ?HC93jÍr?2
¡®f?%r~š&Ug?Tӓꃹ?EÐ3}â34FGL J1350.8+3033?â}íRö"i@S#'©"áÀ9¡%t9ŽÀ<xáR•Ï@F•[œ]ï@ÚöƛZd?°%ºç?·'.~SÔ$@f¡aä÷f@"·wP?ÒXÖ%;"ì¿âRñ©ûçm¿ç8⟜é¿äc²¢)5.¿é'ï~R–P¿ïÿÅbu@AGNfsrq3FGL J1350.8+3035B2 1348+30B?ïÌs—Àü?}ÎØ´Mï?QÎ!Zç?M´j‡x7Ó?uR«Ú+tŠ?{ák¡U?ï²ÁÓ*š?ƒ°Ü_A?GÁ]@Ìß°?Y2N}¼zè?ÓuaL­b?'3
d^™?ï$#)¨—®?'âç\«˜?pçýë²i,?f¼‡kI?—A›Poù?€h¿î~åÛ?ïòY#³ã¤?G¥,v¹[Ã?HŒ'™Ü'?:Ž4Öî+È?Nޖ"é+??eŠ¢EuÙ4FGL J1351.0+0029?ê]ê–â/@Má;:h±šÀ:d­
ê¤NÀ<jm÷È@¡lÅûø4@âmæÎ?ùY}tË?¹•þÀ¡§?õ%b?8È@vÙÑ4¿Ÿf…Åý$Ù¿ä	•ao1¿æšÔ,<ží¿à¨1ý©
«¿ïþpHgwÞ¿êrÀü§†AGNfsrq3FGL J1351.1+0030PKS 1348+007?ïÚ°ˆž6ý?"l¿&Þ[?EÚî›$¬?SûøûÅþœ?oØ»ºÿÖt?'Eÿ&?ï«6ò›Þ?"kAóMpµ?BÛVŒo?UÎ\2v+?"ÇZ‡où?ƒY+C^?îùE	àÁ?…Ò5,¡¢þ?sF¿\Þ!?fU*8‰¥w?œ¯ð.?ƒÂ¥ÑHÓ?ïÙp4ÚÞ[?Z¢·³òðö?Q0͏oæ6?C‹>:Ï?m÷d]i³
?WOïñ04FGL J1351.3+1115¿Ïs†žj@Q1›€#¦ÎÀ9t™kvp À<
cu^P@…oòbü?ý+þ‹‹º?±@¥\ˆ?°¿ð©Jè@¯\äÝdË@á´¼µ¨n?í°çɨU?¹ðQJöH¿Ü"÷ž\¡ì¿ß"S¼ëƒF¿Ôk•D C¿äM~8C"AGNbll3FGL J1351.4+1115RX J1351.3+1115?ïˆÕ÷)"?"™RüãH?V¬
¯½š2?Pü·ZMá?Šõæ>]?ƒhðÒýŒÒ?ïx£Bõ?Žynr~?X¶Z>!ì?f‹íY{š?ŽÅ푾2?‹ãT‹æÞ?îÎ^ƒ~—ë?ˆ­[n¶(J?lfö»ñF@?]ÁYƒ?¡S¨\Wlæ?‡g¸ÔŽ?]?í™s0¶4?'ˆ`CÑ·?< i¡¹m?|ÆPšþ2«?®J¼¿Í¯ù?ÊÐUU74FGL J1351.4-1529¿ïÿë€}@F|SŸºEÀ:}«fJ·´À<`š¡×U½@­ïõEçÁ@ÃÙß?Á»»?™½)Íó?Û¦£Æ™,@""ì¿ÞB#ßX@¿Èš×‡:òD¿ä1YtœU¿Ù"öd ¾|¿ã\YýL¿Üß齃AGNbll2MASX J13511746-1530155?ïNIneð?¢ó³ð?Ph¸àÌ?Dý­gÕ©–?ŠŸV"jj"?ÌÙ÷›5?BèuÂ?†›ÿ=U?CLԐ|×ò?S$ž'à?‰%aüÚÁä?…!Þ*¡?îÛ¥­gl?ˆÁð'Jbó?g±óÕ=?`YíYÖ? Ê"i~ËÞ?‡Ö§º¼P6?îÛ§†˜°?µ‰™Á!?j´¥5uÔ?S9‰¡›? š=C¢Ë?Fï@Ž|o4FGL J1351.7-2912¿Úڒß&|Ó@?օ3±tÀ:J4ÿ¼
bÀ<.43
s†@³Ç­ËÖ@=•!dԖ?Äab*Âv?Ð0š<+ÕF@	¾È'L@K8P©f?å}d¸|߿߀-·É/‰¿å+¦—㷿噹Å¿ïÿúVrÓ\?ïÿÄ`"AGNbcu3FGL J1351.7-2913PKS 1348-289?ïmå•Pá?–쀙ºÃ—?—CJÄ2œ?'ìæû$Ä?z|
FĽ?â½Åð?î7ñ€•Ü‰?¯ùa'­¨?†·Q7>³—?•K"£v@?¦Ó¨ÒŠ¤?§íæê2!˜?ë2!ÑU®T?§jø¬`r?ªi	rpªš?–ÍÚ'?¹:l¼8?¡'vŸ}?ífÂñý?¶"+?"ŽïŸtûm?…Žãß}Eœ?¬â%±$?›šÎ{F'á4FGL J1351.7+5542?éÐärø@M´¥œ[dÀ;•Ùs¤<‹À=<ÖJ$@ŽššuŒŸ?úŒõ–ðqî?ÒÅ%îÇÉ?ã‡/iz@".C	j@´Äî1!¿Ïì\	@E•¿ïZu%F?ì_Î1PÚä¿×álˆ€Ã¿æSÿ¨Â,¿ïÿøþÙå9AGNbll87GB 135011.8+555656?"Ô¯?².=äõ?Ž¦áçÎY?™VŸDJ}	?Ûôv6©?«›š#ÍX$?îVÈÆ,2û?­$š-¸+?€C»_G>?'Ù'ý*X}?¦'"Åk
¿?¨Uw´J–?ë7…?¦¢kW^?¢µBâkò?"ïÕÊS@p?¾¦Ö
Ð?¤(3»ZÄV?îà×Ôb?×ÙW1.<?‡9d䄻œ?`N5ÏI?˜HSzž'?ƒìo>GŒ4FGL J1351.9+2847?íKˆd=a@S"T6¸ù±À;' ŒÒáºÀ<î%ÎÆ¢@Š·ÖpŠ?üýŸ‡Ü?ÕËÛø8á?Ìmñ	Â÷a?ø¢³ôŽ²¶?ÿ¿iÒ~¿ï¤«{Cm=?ïëu™àv¿àkTñ¿Ðü¸''ì׿åévP¿5¿ïÿ'R}{AGNbllFIRST J135154.4+285007?ïªççi§<?Œí]ÓÓ_´?QüێŒ"?KÄãhC'?ƒj³Ä¬ö?Œ7ÄO)ÜØ?ïs'tã!™?'ʪe0ò?VÖÂ!cÄ`?e9J•=U¦? EA…ˆ?i[0›'?íÍRy?Oý?—›Ó8ê?ƒ¤Î¨¹ê?t²à%ç9?®A¤Áܼð?•F_Ü#X?î·°yìg?‰pkÄtâ¬?…ÅÑøCý?w£íå\O?ž'cގQ?"h|Ã÷pk4FGL J1352.7-2742?ӄsá½äk@@œ°À&ÌÀ9ïHk©œFÀ;鼌ã©@‹¥ÝIǟ@M_Âví?ÁlÙ݁zê?ÅPžéd³@é¾àzÿ{@]¤í_¿X¿Õ8~âHN¿èJ€Â2?¿è.ewS¿ë@˜Á­^ó¿ìKt½Âè¿Ù¿†ÞV&AGNbcuPMN J1352-2745?ïJÿ Ámª?¡ùØMB‹?(ºF˜k;?"äËO¡Æ?«º¬X_¹?"3_ªB§Ç?ïª+"?—[r"Aú?kÕ	¿,-°?ttÙvW?œpW˜µ?""Æ›¸È?î+zTbÚÄ?"ù¹ÙýD?‹*kœ9¥?-ïÔ	µì?¦}ÔëEp?Ùââ–è?í»ÌZ°ï?aµÂAt?\àg˜^[?u'‰uÂÆ?¬l;
÷È?Žj°Ø+¿4FGL J1353.0-4413?îá™9;NÏ@1D^=¢ø¾À9u –
À<ùée‰È@9€H9Ö@cZþSW–?²¹'©gB?°c¥kßÍ?ü6~â^.Š@õ¾]ž@È¿ä«KÞ$ãå¿Öì@Ûgo¿ãýMž"[¿âgT"*d¿äÌ~É3»¿ëZ0Íþ%4AGNbll3FGL J1353.1-4414PKS 1349-439?ï…RG<?…@‰q|³€?Z÷#wk˜?R¿ØS•?‹Z†ÿ\ƒ±?"½Gygð?ï`PYæ?Ûôcuj?e•i)íÚ?u"ç¥.K?'F.Þù?ŒR)È'~?tD¡ð?'G4¬î†Ä?~ze˜êŒ&?tE=Vw
N?¤¬˜l?ŒÜDA{rÐ?î™ø™=Œ?…m1Šzª?ì;qÓ	×?s窱pý?ÊÏu©¶?€¦Ê+Â6Ÿ4FGL J1353.2+3740?ìZ»ëS¸@RPñýÞ½À:øªÇ¿FÒÀ<ºjÖ7¯š@(YØ8À?þšþSW•é?ÑK,¹œn`?Å<EÖxó?ót1ËT&É@W9°$ö?ïù¿`}™¿ê:'¦.(¿á hUSïk¿ÒgC±Ý¿á¾Ÿ­¯Ñ¿ïÿå=†ô&AGNbllRGB J1353+376?ﶽ|M¤?‡ä™k]M?Ebï=p ?D'oFqà±?%!§ø¿â?‡µ=2f?ïˆ'¡Ãaü?‹Òè	•‹G?L›I0Jnn?Y «…éá3?Œ,bü"ÙÏ?Š]C;½i?îõ{k9?' >øàþ?u"ñÅ(°?ešÏý½¯j?¬Ž*'×b?hÉðNñ?îî+ËMk?ƒ®ÃžPª?uÓÄ2ZU?d 7}]ò?œÅ–ÿ½1?û`"£x4FGL J1353.3+1434¿ïÿ©\ÉôD@Q¸«`kz¢À9æÔø³À<e¹@þÍÑ@ !‡å<@üæb I?²˜8_[Éï?TrÈkáqí?¥(æ~#ÇZ@
»Õ§ç»?ïüü_·u£¿ä}üàeÛÒ¿ä,u©ÐH'¿â0›©>R¿äa߃ˆ¶¿éfj˜$N"AGNbll3FGL J1353.2+1435OP 186?ïÏɝäZ?Õ\Ö,¬¦?9M°
…cí?64'fÃLJ?v†V
*œj?B¼Ô8?ïªCvQ"?†$XÅó.7?C¾Ðù"C?S°oaõw?"=öoœÝ?"Ý&¶x®ä?î×ÄÁžÄ?¯Œ:'Ó?iùۏP†'?UZÛ½ñë­? ä-*{[?j°ÁÕâ?ï«
䝐?kÆh nÃ?fý°œՙ?S}C¬µT[?~ú5c7'6?g»äô9#4FGL J1353.4+5600?æìï'HKý@M…çÀn¹À;A£[º:úÀ<ºŠ´úH0@ä4µê2@‡"ƒ¸†Å?ÃÙ¹"ÆxË¿"šmÚÎî?Ñɋ¤¹]Y@3=gµj¿ïî5'˜Ì?ïíÜ|m8è¿çl]Á|6²¿äXb—¤Í¿àƁŠY5¿Áè›_lw"AGNbllRX J1353.4+5601?ï¬m"QX?¦S½d罐?Xw3g[ÖW?6þ"­ß¬?Õ×n@.ç?¢èÊ-oÂ?ï¤âoã
p?…A óºÞ?CŒØEª°£?\¶^ ?…Ž–'áù?ƒÊmŠ"§A?îrKÑ?"²gA?{'ÔÔq~Ø?l?>Ñä¥?ªæ£pÀS ?ŽmÓ3ÞԘ?ïaԇ2#M?yÈ#'?pûv±1ˆI?aãÏ-¶•?
"ÚÞhw?xÿ!0¶54FGL J1353.6-6640?ÙdY›Ò¯À)×⪄£À9þ…¬|ËÀ;ϏÁàá@ ÅÏþ¨0?þÚvÙ{0ù?¬ï܂ˆ—$?_¤ßʚ1?µEÀÂ}i@Èm`€žK?ïÿwD;Ï¿Ú×.(\¿â³y…'¿à?€³ï†5¿×ȱil«¿Ø"<z¯ž"AGNbll3FGL J1353.5-66401RXS J135341.1-664002?æ´§ªÂàƒ?Ác:\ð?päMI·S'?p£pnñüÑ?ÒSuSa¬?Á@BC("•?åÀ,)l§u?ƳTCùÊ?V¤‰†?p•»êV~?ÔiŸ«Ž?Ưîê¡»?æ"µWSÍ?¬¯Ñ£/Ÿö?—ÆXr•ûa?'—œîšöF?Ñ]}'ø±?«=™o:h2?ëXƒª<ÕM?¤'*D»C?–C27Î<?ƒÆ!'p˔?¿«-b?£høÜn>4FGL J1353.7-3936¿±/I c¤@5±¶€Z-sÀ;Ȃ—õT«À<ØøγVÚ@"´à®ø{?öĺ|h?Ú&Á HàD?Ú{¤üۈ?úµÄ}î@ø‰*
Àx?£!¼'õ
¿ïü˜!I{Ê?ïþ±¶ÆÑ
¿£×*©»¿Ñ³œ¾ß¤¿Ú€~ÀzYAGNbcuNVSS J135345-393711?î5
÷›ª?¤FÝ÷f?|¢‰«È‹[?ô7S™*$?©ÿPÌMÙ?¢ü<á–9V?î†ü͜ÎS?§!ÿ'#~Î?sö™@D«)?…êžF€u?¥_þ*…^?¤¸ và¡??ìMÐ]ó¥g?¤G©¬ák?'Ë+éÅj?qÐøEB?»8­Åœ?£œIFQ?ì½õ"¥-?£/˜xrß?Xd½q?T™-Tì«?¹¯ÝXÏ¡­?£-	OÕE4FGL J1354.2+6934¿Ö]s±†(@GJ»˜Çâ'À;9‹n]«­À<⟍Ï`ü@ëëêÊ8É@Ñ·Xâ?ÕlEãäìS?Ó`;^ÐÅÖ?ù|ÙÚÒI?ý€ÌC:?ïû:~+)$¿ç]=B€®¿á¾-,ˆõ¿çiÆ×p•¿ïÓ9ÎWçH¿ï*èáÖIAGNbcu87GB 135252.8+694626?ë?ý»F,J?¹R¸ùòß?‡É–'±Ò?ˆõ¼ ˜£÷?Áƒp	~#»?¸ÐͲF
æ?ëÄÖêrƒ?³í~`¿?Ÿ²Ì×'â?M|úýh?¹ìÃ9:!ç?°#ߎɊà?é—í© Óú?¦7Fc¶+?±TY)Žøñ?˜ÚÌbÔ?Àöĵ3ž?ž÷|—ApŠ?ꌄ3œª—?¤Ìî`!y?°cŒ¡åÍ? 0;9à	?»8QÁ5–}?ž"柫xË4FGL J1354.3-0206?ï`´åi@L‡çB™Ø"À:bÑÜFwÀ<+Z§ƒ@;ç¿ÂMB@\àž:é
?Ғ	†gä?á%'`À48@×WŸúë@¤R˜(U?àÒt¬zFî¿ák™v^+/¿é•1 6ç¿ï¬ÖøŸ¹n?ÚUÛ>T¤r¿îû¶úÓpUAGNfsrqPKS 1351-018?é\6ãÑÒ·?Ã}Ü÷I?´÷•)̓?µvŸõ?ÀŒ(¦#ÎÙ?¼€wë§<?켋Qâ[Ÿ?À‹÷ßÜò?¥Š¡BÙ?¹•IFõÙu?®¬©QÀ+?«u~Õr2?ã׬›®U?°­|h{3?ÃñÚRy¥­?¦iΐ]]E?̯s>Îþ?§Ùz'—?íÀU™\Ùà?¦'âN÷ۃ?{•'}
9	?€Ê©"«?°D½H]w?¥Eq÷;ˆÔ4FGL J1354.4+3707¿—í<¬ú7@RWRÁmóùÀ:‡à	Às"À<"Ûá<ÆZ@ãZÅô@"?ÿ¾•·ŒÉ§?¿˜kàè|p?£\Ðeˆšï?ås|>ió@¦IÐÙvÔ¿ÔWQ?ãšÅ?ì¤'D`'¿âƒ''g›ñ¿áÞSÝͦ¿ÜÂ÷¡aº¿à蒀u±2AGNbll3FGL J1354.5+3705NVSS J135426+370654?ïjxB¹¯Ÿ?‡ã%Á?oD.b"|H?bÖ;ôë¯?ã¹y9?…¶!õi?ïx©ÂtN;?ŽJ8'pkÜ?X''2"S?d®Oàÿ{?ŽÒ*~¥?‹ºQu(0?îB3¦;?g&–
´>?œ/9@	?ošÈ®ü?«ØVß͛:?‹à%ns$ê?íԜÛY¸?Ž4Óåf?›æÿZïS?…¾ºôPæ?¥2¾Ê¶ÿK?ˆ'$Ï[4FGL J1354.7+0623¿é©ù@ѵ@PøôsÀ;EÖÌ*žÀ<¬Kä ÷@ 1´XÛ?þÐßìdAÉ?×¼.Ääv?¿L'Jò—?ì°ç~~á@†,ÞZi?뛽˨	Ÿ¿ä	"ˆÁB¿à™"º\‡À¿ÐÈøÂI?¿åøžï!‹¿ïÿø]Ê5™AGNbllNVSS J135444+062249?ïōSÙJ?w‹¤Ô™P³?@—ýõ×,è?9E²Ç=ò?{&qXtþ?vë£n/?ï,Û@u?•á	¸F?W҇lµÇõ?eˆ»õq²º?˜çu§"Ý?"Ú©oÍǛ?íûˆŸu¥†?"©+<Ӝ?r³¿\ã+}?\JG—N­:?­ðþ	B?'çGüiê?íµ‹Ò}¬º?"øÕ/0h?sìÉnŽ?lbâõ§Ž?±ßE?"|¿€´:4FGL J1354.8-1041?ìÁë²Áó@H•žbV6mÀ9y˜éåÀ;ÿä[^Ëg@n¥ÇzS@*¬azŠ?³Æÿ> 4ú?ǚ}DNc@#»@³Nw@›°´é+R?ºªÅ»ám¿âÈ}}`Þ¿äù— ¢‰¿é[ibš)¿æ1]À¥w¿ç± @Ò®
AGNfsrq3FGL J1355.0-1044PKS 1352-104?ïrxê(ö¾?Œš†ýÜ	N?z€×qÿG?wœqB%?†!Y¼ÂÅÑ?"lÛ>¿-?ï|‹þ('?Ž×&ûÉ3N?Oý&Kû?cϪ±?ŽÜ
Ÿñ­?Îo¼–¹S?íÔ=¸Ö6?žt9kO|_?"p®Gˆ?‰ÝtÎr"?¨ºì*¿Í?—þ× 0Lf?ï°…ôÞ?i²?ÊÆÁH?]8±Ðæ¦?KJfêè?€W"¤fÌ?f»ž‹_b4FGL J1356.2-1726¿êV³œ`Y˜@E]ȟ@¢‡À;ùÿ4þåÀ=2Pµ$:@ @ԋ2"½?øóy	YÂ?×[	T<˜?íGâb
a-@
VŸ¸g?ýø8RÌ+¿ëÿÝe¡D‰¿ØàEš¾Ý¡¿Â¢HڏX¿°¹€AS²¿êêË»TÕD¿ðAGNagnPKS B1353-171?è>å…Z&?Á#y"œ?ÀÄËhLp?¶³V2Ç)?¼=®^…ï?·ü1­ÄV"?à'>=·ñ?˼‰<8S-?Ó󺈨j¼?Ì^[‡n?ÅϑúXJÀ?¹?±5‹í"?å"Aû]Ò'?²)aG¶'@?ÃkÙ,?©Ê°})¶?ÆG\O?­­UÝYÓ?݊ò°´cÄ?»È`¬ÕÈ?Ñ°X'w,?¿ås€{ôm?ÐÄ´½Ô?³µjUÇÏ74FGL J1357.1+1921¿îÒ[Í0Iõ@RBä¸{ÜðÀ:?
€Œ'ZÀ<^gpQ¢@‹íi>]@ý‹{ɤú?¼¸•!(³l?Ž3Š4æ€l?Ç⧋P@
6҇v×M¿ãv֋'oڿ䜝Öj/¿ë SÇþ0ó¿åèe¯‡A¨¿ð?ðAGNfsrq4C +19.44?ïö»!˜é?a-¯ïK˜?Bgýx´Æ?Ayüïü¡?B«òr#¢
?`\fô¼9Í?Û0?'àO$ÿ£8?Q.žÈÚ5?g'—Hz¾Ë?ˆø¼ÕZßË?.
$=8Ù?ï
H½Ï×?''Ë8?r‹1dw(€?eû<é"n‡?šíî?€½7…ò•¡?ïÜKàI?`kÂîW­•?Süî
"?H¡"`ËA?j(¡€ç±K?Z‹Ž¼^"4FGL J1357.5+0127¿ÓŸ2ü'ÉW@Méä¼­šØÀ:/½¦îíÀ<V8‰´IH@Ú;ƒd@ü wnÌ?Àx^ õ-"?Ã%›Åî·@oPóÇ
?ÿî>¯h7ø¿ëïþ€#&?ï	þ¡[.û¿ãOˆžŸ'Ø¿ä‰]aZ
¿âàsr¾c}¿ïÿªÅÝðAGNbll3FGL J1357.5+0125RX J1357.6+0128?î®Q™°;?–=é¿;Š?'ÆJÌ.þ?Žƒ?½®û?˜o'Ä#é©?‰Àȅ1PD?í_Ï~n»û?°Ô—ÏLlI?—ÿ{'K h?¡·/îjsÎ?®JOîp(?¦î­cã(&?ìX#5£Œ? Ô!yFp?šÉ–{P1¤?‰÷4œ¡je?¶Œ€´%?˜º>ÇL?ècz"ê ¬?§|–Ïfˆ†?À®It›¾I?¦n!e§?»‡˜ws~?—ácADt—4FGL J1358.1+7642?ÉLÅ!ÿüq@CãŒCoÁYÀ:ítãìÀ<¯¾5ZTà@ŠÍ©ìx@¤%t:?´,Ù&ø?¦ÒU¢ÉÄ?ðjâF±•9@wûmŸÙ?å_¢!¨q¿ß›j$ÎA¿äýýâŽl¿ãÙwÕúrø¿êþMxX×2¿ïÿŒýÿʦAGNfsrq3FGL J1357.6+7643S5 1357+76?î٠鱃ç?±G²¹Íþ?t¬a«ÅÐ?¸2ïÆÉ?Ÿ°Êi䑜?¯¯gc?ï©uDå
?ƒ—Ú#¼yÿ?GPd®?X?]¾Þ£Ì¯—?"2IÀpb?¬ü¤?îэj$Ê?ŽD…ƯŒ ?xc9H0ë?pétK#Fw?ŸÆ µZ"?‹;¨°Áöü?ïâ–,‹š?VÕ¦'dõ«?[ÀÆ4
i?I[AZ¿«¤?`¹mã[?N§7¢l4FGL J1358.9-0703¿àò$±Kx@J
At>–>À;Ž²‹Øæ·À=þæ$Œ§@&þTb`?ù(
Jk^?×ÉÔ_hEd?çN—rwì¡@Æþ÷ÂCÝ@mI%7òá?ï­àx{;á¿èÈ¿AHõ'¿Æj!´Û"¿Ä³w¼$3¿íQÖ¤¿ì‰pÃõ8AGNbcuNVSS J135850-070403?çMÖ^Åý?ÀÒ®ö½´ù?º},EÈ!?³®‡Ú]Ð,?ÅÇé\bú?»RhWlò?êcʎ-uv?½é²1f?°¹ÎãÓ?²«¸tY^?¼Ññ¿°8?²ÄJëR«?çåƒhxq ?¯ìàméã?¹¤Jé¶Ö?£¹%½[2?×ÍU©^?¦ãl^àòÐ?é­¾›,Ó?«"ªí?´y—í2ȃ?¦b³®IN?Á|}ùès?¤tR!¦)4FGL J1359.1+5544¿æätÜÿR@Mq%F
¦LÀ9¢x>Õþ¥À<Q¸ÕŸf@v$4Õk@ã¼ûžqp?­7¿^û
'?¼û•0©@@c¦@q	@Å?à?Æ?¿Ô÷íwg?ª¿ã=]º¿ä<Ž@ @¿è«þ +ï¿ì ©¡Nš¿ßáŒAÂB/AGNfsrq3FGL J1359.0+554487GB 135720.6+555936?î]¾KSÀˆ?©b¦`a?~š'G_9?{«‹g"Ô?¦PË	;®?§XȈ;#ï?ï/§6'…Ô?•*y¨çõ?dÇ<C"ö?pYU¹4®V?—ŠÀF&ÒÑ?"u܌§?îJEIÃÒê?–·èZ§?‰f¬Yψ?ˆP7Ø0)…?£ø
•é ?X7˒Å;?ïBc+,?{Wô9>Š¢?ƒî*$è?n±¨ùú?‹Š}ª?sD±O?/D4FGL J1359.1-1152?ÔOp³ÞÌ@GՊ"-QrÀ;ًŸeÀ<ÏÅ'iú@#"ß³Y^@?çK¶ý'¢1?æZŸRk2?ã÷{a .?øȃweR@ùi'é÷Ö?ïñZJÏ1¿ÍÏã؂µ¿ãßIÈ¿äøRAkZA¿ÿâm•Q?ÊxýrñºAGNbcu2MASS J13592131-1150440?ëúÿ³ãe;?»O"ȋ?'w7áA•'?"=z&L?»Š4h"pÆ?¹ÆDKDR?í#fºìê?¸¢ßǀ?"¼èÉOî?¨ÿK¦Äiz?±µöGŸÅ?±Ê Ñ]?ë–û¹‡W?¤)È0»J?šø°™œg?ˆÜtkPU?¼‰ö
\kˆ?¢p"=•B?åTÛÉ?Áü"O?\\÷­·¾?mÃäâ•Ç¸?ÕÖ¸ìðÀ?ÂʵŒêg4FGL J1359.4+0202?ì<'
öló@N'¼U†DÀ:"R:_w_À<Qhª
…@ ¿'țæ@]¨!ò™?Ëæ	³õ?Ï؎!yd@¿2½ÂmÎ@Z½Ä³Ï?ïÎÃè!¼é¿ä…Õ"ܤ¿çuM‰öŽ¿áÉ/ß@¾¿ïÿ×,uª?æ9i"ƒb¡AGNfsrq3FGL J1359.2+0204PKS 1356+022?ï†fÀ1U?"åˆrÄ݇?i$ƒ&yv?bO‰ô˜6¦?ˆ/*]N?'†–^Õ?ï+¡jz?™á®e÷5?h×3Ì+?{IYr;ó÷?š?«×—/?–TP6¬f?íjˆÓ]u?š
KË
g?"×A¢'ì?"íÁù$Pƒ?¯kÑù.ĺ?"g43ß8?îèm•'\?ˆ®Œ!Ób?€ƒÎ+??pґ[PÞ:?šê‹f"éä?"äœ
6—;4FGL J1359.7+4012¿…ø͞¾M@Q°–»™À:V²w¶ðÂÀ<|J{NTø@^VòU'@ž[BEõ®?ÂZCBð?О饴¦@	<J@•òE@G,íHî0?ï÷6Íòfº¿Ù«"}¨¢K¿è>Æ¿—…¿ê~€¿ê'•¿¿ïü€s,óAGNfsrq87GB 135731.7+402612?îäUŽÎËO? áL{Î?€–QÎ,¡?7ôkÍ?›-ý?Ñ?ža3¬‰pÙ?ïdþ©çNé?"ÑÆÓ&?aٌxÜOg?x­m'+g?'$ù3ú˜æ?¥ûȬj?ì?"ÞV¬?¤¾,¹Ø"5?¥lR¶d§?"Â÷›ù7á?³x"ãïi±?ž Neñ?ïeî…ö2Ñ?xDqi0?"çJ2\Ñ?n¹²ñl¤?†ºjÝZ?pQÓ:W:4FGL J1359.8-3746¿îÀÞÿ¡­²@7&=_ÜßjÀ9…/…(ÉÀ<¨a³y@ºYÀ7@"ý°šg?¬ªþå´á¿ 3ÀîÈ?ó@YÂ5g@N}âÝ?â{8 Z}û¿àr·!ê¶m¿årÚ/­m¿Úx›)ñì¿ÚÄGÃ
0j¿åÅYa›AGNbll3FGL J1359.9-3746PMN J1359-3746?ïÊD7®d?sVòNF?CÝDu,&È?;¢(bÀ?xb;šPÊ5?r\ýÑ•?ï³Ô]SÑ?€ýÕóS²??ùX‰yµ?Lˆw/Çì?'÷>?€&6ÂtK?ï^ãJ£ä?"$%TT€?h4Z¬]D›?U‡) ø_?œ
˜AÛ?ƒFM›?îÈ£›h1I?ƒû5)s¹?rCTìß#?[DQ›˜Å?¡-[«ìï™?ƒ‰‡³Àõ
4FGL J1400.2-4010¿í¤ÃÓÌ<Ñ@4Ðù;À oÀ;ñ՚ѨÀ<Š¹æ@;Y@ ÐXz•rn?ÿ"<jÿR?ÉèxyäG"?³ÿè¿,âG?ä¢ÿñ?ïäOþ΅<¿Ø—"{ªñ0¿Úki¦Wî?ÞçÖyô¹¿äh M¼¿Úd¢Qy¿á'Y
]QAGNbll2MASS J14002208-4008235?DD?©ù°ˆð?eÁ`?càœXÿcE?­õEâ›P?¨ã*s³?ìzF;[[?ºEK¾ïö?'},cR7? Ú²ãªÓ?·ŽƒLPž?¸Eoî¨þG?íhq6ÂÀ?•å«mõ?†TÑûmw?yëÜÖgÌ?±ñÜ.ú|S?"}"d}Úo?ä؃¾ª¾?°¶AÈXˆ?Ÿ
n´<r?–†öê†T?Ô^VÌûf¼?°é4<iW-4FGL J1400.6-5605¿°;hÙÐð@õ†_*2À9 syt`$À;¥›/›Ï@§ÍŸ°‰ö@
œ \–Ú?µ@1ôCß(?·\<ìÅe¥@,Gõb@i‡-0e?ïÿúŒ—Ó¿å:ú!™­¼¿è.[}T>œ¿äǸ@MÍé¿åyÁg‰&¿ïÿܞüÚÝAGNbcu3FGL J1400.7-5605PMN J1400-5605?ï˜3Ð<?‡3p¯Œ?Akæ=¦W?@'X™Cê?ˆÜM›jvS?†Œp=Δ?í•Â¬H÷Ï?´Rrt[Ô?[†h"Ùôt?"ðº'<Á?²ãÐû¤Ù´?³ï¼Ã¼®›?í%hԑCA?œƒÆ$?‡ìÖèô»?€*®Ô–ïø?³×~WT?˜òæˆLá?î}ÚuÜEÀ?†ß7Ípè3?zðóêM¾é?b/$Ÿ¨#?¤Ä:$ñì#?…AÛ\åï4FGL J1401.1-3717¿èuehd˜@7†Qm°ÝƒÀ:ˆWUQk-À<T"ÿ®¡i@ ÆK¢ë§Ù?ýJm\#íE?ѽH WÎÉ?»®ÛJ>´?ìÆÝ¿¹=ú@©ùŸ"®ž¿äp]€c½•¿äÐvH¿æ•§œ'œ¿È/Š1FÉé¿Ýê …0«ï¿âÞë}'üAGNbcuNVSS J140113-371757?îwÉ»Î?œk²¤ü>?Y6{Ñ-$q?L[*A¬i?§¹¯õ¹´ä?œI·ØG?ïç´­ß?œ›âò¶?]ÏðTÅyÏ?i+Ø]$;ª?¦
d÷Èv?œq7ΰò}?íHä´Lö·?–[™ä^?{5…Õ‹?h°oÁ&]2?´ç/ìí?"Óºåãq?ëõ˜8}¸¾?Áæ9$íQ?u_î`†¥?iOAøTP?¿X=,1¢?Ò£~nÛð4FGL J1401.2-0915¿í°òÚ0@@Hïâ£Î¦ÂÀ:¢nÚ©.bÀ<''¤{u@Í>¿‰È?ÿæ҂s"?ƪ4Üօ2?ɗ(¦w!?þó(ýOL@ë8[犿ìî`e›eL?ï÷`Æu¿äò–UAzõ¿ÜPj{žÝ¿ë±Èd?¹w?§ŠÈñAGNfsrqPKS B1358-090?ìðF½"ê?¶PéÄø`°?›ÔÂ1?"òÝ«Ÿ•?¸?H™"án?µ×jÓ$?îÌáªÓ˼? Š%o¬NÍ?v'±(ûŠØ?"j>V9¡? _-£ÒÌ?š×md)?ì¢-ü¿Æ¹?œêÛó?—½m.Uj?ˆºi±ù?µ, ¾¶4Þ?—E†ÙÜ?íXó䜴?"9L^¥0?žÛ|û?"hcF5[?«o«³ð?ŽÁ^\~ñ4FGL J1402.5-1827?Û?
#fÙË@D¡¥q"À:($5inYÀ<(]yWÚ²@
«)¹ã@·Mú^ÖO?½¢³ôŽ²¶?rõoÇýÊ?°öÌz—uÓ@¼"K̲ ?ì×aPQý¿æŽÛʖ'¿ã˜íl…¿çŌÁïÏ¿ïÿþó…õ?ïÿÚ €AGNbcuPMN J1402-1825?ï=…\lè?""6èU9?~Uþecr?zêfñ×k?¹ÔÙ:J0?q…S5ÀH?îÚºÇVí÷?¢?QZõù7?g=frÝH4?tÃ!?Ì÷? à}#cL? Ø
×6Îþ?ì"ùšh?œûàëÑ3K?›Vº‰'—W?‹Ìœê"#?´‰ÉÊææ?–#s¢!<?î獉H4?†Rú´'Κ?"9-׬?viGnë Ë?˜ñÞXIš?€  ó‰4FGL J1402.6+1600¿ë<aÿ	Ç@Q†	€²BÀ;-Ãք´À<­póˆ"@ …H~Éà?ÿj`Æê4½?Æx"%çEI¿{)øã0Zt?´¹øå¬Ã@™'6¿ïÿçÁŲ§?ïÿÿ>¹ú¿ëbrϏ¿ÅÚñéû%¿Õ0ÿ;ßÕ¿ç£ìòù‡AGNbll4C +16.39?ïÔtWèy?yz¢Ô"?3i¬€5É?5_Ððúû?t9CÀ?xhH%äÙ?ï²2‰µ·­?"®®ås`)?=†¹B痖?Q(ÇS¹^ø?'‡'Èz×Ò?ƒeÄÏêyz?î^4pFÅñ?rÉ*ün?nN‰rÆ®®?q/ҘC¾^?¨7Ðdg5ò?Ž.¥Üýö?ïr°|
¢(?w¶ön³?^]‰O­!?Tz'\ªÿ ?ˆ/Ò¡Õä?v@"Z­;o4FGL J1402.6-3330?äŽêž;aL@;GÜ7£ÛÀ:˜) ã9÷À<kiA@®[®ýY@:9Å«â?Ò¸µ¾"N&?ïj-›C¾@	¼=h@[:@1mD&¤?f¾uœ¿¨»¶OùC¿î!3âÂ]¿â$A"HFÁ¿ïÿ••_x?ìѹÁ,Z§AGNfsrqPMN J1402-3334?ìL‹‡§:f?¹;ml2§[?³¬ ö»úë?³ƒ†ÄW?£ß˜c¿?§O5'å½ú?ÛPePLßõ?Ñ6®â÷09?݀'½&Û?Ñé8pIÃ?¼½ËÊsäÂ?²¥mCº?é""Bé"?¨x¢gb	ƒ?µ"2ç.>ü?¡[ØV.'?ÀäÔO]:q? A¼:a ?ßÇyn¸b?ÆîB…¤
?ܱZˆŠŒ‹?Ç& س;O?¬9`E苀?œœºÃ懲4FGL J1403.4+4319¿æN©Œ3ˆ @Q
ðoiDgÀ<#01 3|À=$P%"õ@"…–VÄ?÷"Âkðê?×û .y?ÍЛ¹Y}u?ù´@€#@¼&‹*‡¿ïÿý{ÁA~¿ïÿÞ°ô)?ð¿âH+üÆ¿ÂDm'ºZ¿Âd5^±'2AGNbllNVSS J140319+432018?ìÀ\¦5!Þ?¿'¿"v?eA•ö;?kõE3âƉ?¹S¦ç6?¿aj0¾³=?î–ä°íI4?«®f®Vy?l??÷r\<?¸Ç…´á?¤ÍÀñ´Fû?ªx6QÅ
?ëÚ9dLV?£|Sjv?‡~ •u¬?€­5úãä"?¾Mv`Êî"?¢ÐÉs^&Ð?íãiQ¸ån? …U2+?Dö6QhÕ?IˍMRÝ?°ºÉ–à?Ÿ÷U±®ZV4FGL J1404.8+6554¿œÊ÷ŒH@HÇé·¿ŽÀ:ªøf®‹À<Ž~(א@>Â?Ö?ýÕ%t-Ï?³š³Êó-à?«Æ¥bÇí·?ö7yU@
uèúÕÉ¡?ï÷€—9î¿á"†?IÁë¿ÙŸ:":½k¿Ü‹‰`'eC¿ás°0´Ó²¿Ùl#"¯¥AGNbll3FGL J1404.8+6554NVSS J140450+655428?ïä<Æý:?`—Wᖿa?5Ój71x©?*^i$äØ`?i̤˜2?_!AO–ó|?ï©HûS?…œg¸ô·»?@,]†ÏÃ?QÚOÛéþ?"¬6ø¨¾'?"ƒIÊý}a?ï.J	ãj?~¥Ì¢é?f6"Éîî›?`äiRªß?—oî5µ	?|6ĹZO#?ï¡~»Çœ5?jAN2­¶?c<Ãv¦Æ?JtUB‰F»?'ÑL;H¸?h,µ¥düv4FGL J1404.8+0402¿ãZVb¸@N€ƒ§ŸíÀ9éF¹!õÀ<MÁ}ä1@…$1–¬@b"òB¨?³pbé"='?ƒ\³VGú?Ò'!,öX@Qî4P"˜?ïÂ.]á\§¿Ž¬)ò N¿æù­5WС¿Ò=ÉD6·¿æá	/Sª¢¿ÒºBUeAGNbll3FGL J1404.8+0401MS 1402.3+0416?ïrQú©Ü?®h
­?Xá:,ë$?M›æ	ãBå?'­
u§?€â_ŸÕR;?ïƒg7š[?>…7ÁLã?TMè©v²ä?f03v?Œœu:c?‰åÝÆ÷Äâ?î'1Þºcâ?Œ"ª…¢#?tcӋ;#7?dg'Ò<D%?¤Pg¢ò]Z?‰('–Î(É?î­:^š?…d7>ǂ?-ûD`#)?x–Î1@æ?š*Ây"	v?|–ˆ¨:hÄ4FGL J1405.3-0640?ì
ҟ}<@IàU!š"{À:ð¢nTqqÀ<…e®°'@qÛ$(~N@…ŽêéîF?ΠiA#?½ÆŠdó¹?ñ$lü'œþ@tP+çd~?áC"Lx?ïëقgÎÆ¿êÑ¥CñÇX¿ÇJ|ùzÖ¿æä_æo‹¿ïÿ'Q¦»ÁAGNbcuNVSS J140504-064056?ïK/Çò?£Ê#Œüÿ?rӁ+Á¢?¢_.DS‰¦?'j¼œ?‡ux«J?ïE%Èö?"wêÒF0?e£½>šý*?qñM5ñô?"¦ä_
Üz?'›V-5l4?íû¥O§ºx?"@ÏؐÉ?è±ý4L?kÃÛrìep?¬a­ïD±ò?Ž(VËq…?í؈{PS?"Á]e¥Öé?šå‹»w?‹_¢

?¥²mxÄó?Œ—ÊY'õ4FGL J1406.1-2508¿ïÿ²Sézò@A[¾ãÕýÎÀ:Û»}0À<Vºlwø_@,¾yø¿?ÿ–Ù æ?¹'ßV?³RæVáŽ?ùˆ
%ð@
¤íÛ:MÚ¿ïÿ'¥4?ïÿÙiÍy¿ÚÜÜåHĕ¿ÜˆÖž椿æob¬c¿Ö§ayWAGNbll3FGL J1406.0-2508NVSS J140609-250808?ïèýÒÃ(¢?i—uYJ{•?9>­;=%?<pV½d?cÞ¥g/ø?g¡íµýá?ï˜É2O%?†äf力?O®]lo?_¥«þrj?‡Ò͕~­?"u1Qy?ï¯^'£=?ˆ²Ïð Ì¥?g5Õ»?`­¼ha#–?œYŒ
7¦?‡¢øË×0?ï;ñ¿ªá2?yìØOAÛ?w-¶ukZ?`'ÝÚcÅ?'¶ZmIZ?uÂÃq½Û4FGL J1406.4-1654?åùg3*@E,ÔV.	ÿÀ:à翗Z$À<eôA…ÜM@v‰Á_[Z@_±@L?Ææb H¤?%U`?ìæ?ÇåTƒ™@퇂k?àM³¿ÞIMü¸!ð¿à+bùÌ	¿éD5囹¿ã»gêÊ䕿Ë58›ýÌõAGNbcuNVSS J140638-164954?íRâm±(?§Æ&oºd"?c¸&&ÓH/?Y¼"˜L?´Ë+a@$Ý?§Šþ(]™?ï=ÙHÂ?'‰)íÂ?SNåtÐRª?`äìHe5Ô?—a­‰âŸ?'+%éþÖT?íN-zN?"v
CâY?'Ê=ä–~?t®ÖP/Ö?°¼GŒ7šÊ?'#spÙF?îÓ¸ Õ¯?õ)ô‰¨­?lÖðÆÞ»?[<o<C÷? ÷ù'·>?ƒlÀw4FGL J1406.6-3934¿Þ± ‡<¨[@5z9'ÍÀ;2Êo${
À<œ!Äuæ@#14…×b?óòPµû?Ö|¦Ä¥`ø?ÜL³aì¯@ß덂4"@
^6¬j—¿ç‰Ò¡ÍðŽ¿ç/<B¦¿æ`ï. ¤»?Í#£×dÖ¿")xc,äԿϊ"=fèÂAGNbll1RXS J140630.3-393508?ï{Ÿ­Ø­?Ž›ž"Ûˆ?`7P[tÐ?fdz>´~}?‡ÓSr÷¥?‹ö±EW(§?îðJýðmþ?§¬§'ÌÉ(?f™eÝC¡?'àDø1?Ÿ#s ö—Ò?¥«'ì$¾'?í@ôYêW4?o-åþ?pKq¼¹?p¥Äq"Ó?´Xy'}ƒ?œ"'†'°?ìðÆ6JšÝ?¤ÐVŽ°3?QMTfÒf?ZeÆjG‹	?¸4˜YÊ?¤ÑFMÍR4FGL J1406.9+1643?ïÉ='@QjŸDÔEÀ:·í£ùoÀ<'"ͧ¾ @ ÔÇOŠVÜ?øÒó*öN?˅'òP¶?Ì£f÷ÛÄ6@³Þ¿=˜@³ã»¦´µ?ïÜÛ7ɚé¿â} _žû¿º¢>?¿Ðºèß'q¿ÛdóiÅ¿äF a3÷AGNbll3FGL J1406.6+1644RBS 1350?ï‹ëÂhŽ#?'zª'ö®?V†ZB	ú?PŒÔ«B?ŠAžš"5î?\͞æ?ïb$$?"ÑOœí?ȔPQš?d-¦s‹V'?'^´lJÖv?'2¢æÚ-?í¸:/æ?"¼¤ÿ~9?zç¯Ò0?lÙsz}ðU?°½L7"?'eöƒ½lí?íqhçR¨?–œ»àòz?}ÿÊϊ;J?lzêd;?²"¼"Ç
?•î_f+lõ4FGL J1407.5-2706¿ì´I× ¡‡@@a輜$À;oŽXøÀ<¨¼ÆÅKÏ@!jÑF"@Hpa'ëO?¡6›óf¿º'ê?Nt'?ù"ÿü¥?ýôc>¾­?±f£M!›Ü¿î苤äPw¿×0ÄÃéÏ<¿×êäûAÕ7¿Õá!îgQH¿ÇÚÄ\:éAGNbllESO 140425-2655.2?î_ˆ¢ï?£D½NX7?qm¬oð7?iwiW)À??§ÙÉ`WÊ#?¢Ž+½a=?í¸²¤ÈZb?±<'`P¹?ˆÁG,¼g?[Â2?®s%a¯*Ì?©ÿ›{"¦u?í±>ëcâ[?'ÔÐ73éÖ?v:?Ν¸?fQÕÓ¼&?±d§÷¬?'Ö³èe|Y?çÇäª=¡ô?³š&ñ?‡}Á!‹ý ?' ƒLu?Ïh'Dð¸Y?³4ÿ"doÉ4FGL J1407.6-4301¿ï¬Ïô'7@1°§¨PÀ:Êõ\8À<B¾Ü-"@ߗ mˆÅ@Vç_ö	Ý?º‰ 'RTa?®`ÈAͪÃ?ò$ötfj@)¼=]ƒ"?ïÍ€°ên¿×.¡S!e¿ßÁf<J7¿á›·¡Aƒ®¿á'€ãÀ.Y¿ç*`Æê4½AGNbll3FGL J1407.7-4256SUMSS J140739-430231?ïâƶë†\?bVŒcÜ×?<@K¥w?1œ˜…~?i·áô[?a¯CÎâ7?ï´éºÅ·?'ŽH2ë²?=›:õ‰k¿?Qî0V?Øåù¢G"?¨ýŽ¥O?ï!|'Á¤Ý?|ópø‹ï?kxñ}2¡?Y€ža'¾?˜aQx%ƒ?zÅ­'EÆ?ïeÅ¥ )i?uI<cÖ/?[Ë0‡4'z?EXµûJí±?'Š˜C‡Šê?t¿Û³s(O4FGL J1408.9-0751?äAó9•o`@I%ñà'Œ7À8³çïhHÀ;Ls¿ë<ú@ÒèŦ¾@¦Ós¯û?¨g^«Sx?²ßß#;™^@	™>›A:@›¯|¿©Ý!-ÍË¿áFvÜÖ/L¿å¦@q	W˜¿å
ñú´g¿æºy
2ª¿ëyÍ¡^	 AGNfsrq3FGL J1408.8-0751PKS B1406-076?ï‡ä-%vî?"£¼ùEY?JÃroÒ÷.?B7Q»íi?ŒZ½¥!?"?'ƒß1à?œyø©?…=›~¿`+?GðÞe;n?X}˵ˆÁ?ˆÝ
û.Ä?"Mçuú?î¯äýAø]?'g­qkr?|±-A•"`?sXŠ&î?¡kŠƒ­Õã?K²s­m?ïiÝãHúµ?{ìðí}ƒ"?X9Ã¥Çæ?FwºüÅäú?'<Oú¦LØ?{C÷¦.`4FGL J1410.1+0202¿ç¯nQ08@MO@Än&À9Ób ß9À<V/Ñ|_@ÖC€Þ6Ø@óò
s÷I?¶ôN›ï_I?· Täl|?ÿ‹…L»@
ùÇÚñS?׀ät^Í¿å)B™'¿ãï°A{ËR¿Þ{†^(P¿ìèné¦ٿïÿõ4ÊãAGNbllPKS 1407+022?ïm<<x<d?†¥!@­D×?gc/º·¬?\ô–  T?ŽØ$ómù?"ùŸÒ=®?ïe e³AU?""‰‰f÷?\mÔ3Œ?s´gYÌ(?'•"ÌTœf?£	áüE?îÆp
›t?‹«ò>Eµo?"t¡,Ò¾?€´tœò­•?œ÷­É#0(?ƒ6"@^?ï&¥ÓBÌT?—JÁiU?…"±Ô*Ÿ?qOD/í·Â?i?¾¼`?uX¥H.‹ã4FGL J1410.3+1438¿í¿f‡@Pòy»­À˜À:aps/¢…À<[IŽ¿@Vp–ëêI@ߢ'g?Àe@ ¬s?¼ÂSL-U#?ýPÕ©²ì@`dÚEÀ?àý®(`q¿Ë¬Þð»¿^¿áƒþÿyó¿á¥?à?Æ?¿âlÁâ
&¿ç€[AGNbllNVSS J141028+143841?îÚó:ª?'L:ÍÌë‡?xFo$D!?o0àd¾œ?ž¬X‡¢T?¡ÈÁéb?îé-gÀQµ?˜
	/©cÞ?poœ*—t‹?uâ.]\?ž¾kýOì6?•¿?Ú&Ƨ?íỸ˜¤®?'Ž!x÷/Í?ƒ6f.Æú?sò‹[uµ?­¶Üê^?Ž.kh;™?ì7HÑÀBÐ?"™ hðÑÎ?¢˜¡0—L?‡IåOœ?´ùhðåÏ?Ì¢£…ë4FGL J1410.3+6058?ïå;Ӎ'¾@JÏäy'¼VÀ;ø|²F+À=* ë2¢@"o±UÍè?õf|¡;N‹?ÙS¸ä¸{Ý?˧À£ÉžD?ó0Ì5Î&@‡¦<•1«?ïþ—Ô¿ïö({ILz?éÙl€OF¿±R á·j¿Ò|ˆÛ—¿Á7»˜œïdAGNbllRX J1410.5+6100?ï2©¶Ç«?¡ö›-÷Î?BìèÁd÷ä?SnqÞX?‡7Åä?¡‰é"b]?ïRz²³ú? 	¾ dYi?Lì
ôˆ?^«ìC…˜m?"ÏÄé9à¬?Ÿ_Ýœ—†?ë(Üw5·s?­;PM6›ä?u¿·\O?uÈsl8ÃL?®f®=Ä?­"K_{?ï˜X–Õ"?y4î<‹-?*.­¶_'?/,®ûßÃ?‰"Æøÿ?xç¯ß÷[Ò4FGL J1410.4+2820¿é[hd©‰@RÿCAžÀ:•ÝÞmAÀ<£xOYÚ@ï£ö¿ºk@
·Üz¿º?ÂpPJUl?»œzŸƒh€?øÂ^™éJ²@#JæX9?•"|¯‡¿Ôs£eË5ô¿ßéIDÂ|½¿Þ'G۶ʂ¿æ3OîTÜÑ¿ï´
ɇïAGNbll3FGL J1410.4+2821RX J1410.4+2821?ï8Ž›Õ÷+?ŽèãPh?bxm€Š§3?VGˆš<G?–ŸÕ/ÅÁ?ôJNë¼?ïsçä=¯?ŽáQ¶ÍG?S3½GO6£?^æÉX?OǨVÛ?Œad<«{Ï?î«7L}˜?‡ž;¤'{?tö…»ËV?f¹š±Rû½?¢ÉŒgwm?…fLÕOŒ²?î"TaLH?"Y¥¤2?Šb–ŒÇŽ?pJ‹¹ºô?¡"4AX	—?{m\Ó4×4FGL J1410.5+6215?ÛÚ"BB@J@8ÅCÀ;k
Çhß½À<»§œ'›ž@ŠK—Øú-@47yéÑ?Áe»È®¿º·¢™œ?ûz	Ì1œZ@´)Q.?ïÿƒVR¿çÞQ"'¿ãŒÝÞíᚿåÉ3 @|È¿ßÐÜH*¿Ò/ºÏÊ-AGNbcuTXS 1409+625?ïƒ=ìô?è"³k?r%±Üyî¹?m.BñÅÿ?†-%ÂGËx?A¯øQ²"?îk©@I=?¤'ý…fOÎ?x6¸Å1³>?‡ÓšBêäm?¦>"âɵÕ?¡´ÜP{´f?핦Åb£:?"®ïÕ÷É??ˆ!T¹¹s?x¥j݇¸?°NŸ=³·Ô?'
›MÜ'?î¦#å™ke?Î‹f'Ì?ƒWžÙ­æë?~ŽôJeÛN? ÇÙïýÐ?‰'Öß»¡y4FGL J1411.5-0723¿à'À긽@I3ÞÑ·À:ŸÆh.½ƒÀ<]ùú,h@ ó¿ÕÃk@0«Ü'<®?Á¶f2¿©b_¤3@?æùžßY—?÷Z®Fú»H?ä¥+"˜†I¿§Ež€ð;£¿åø}àU•´¿Ý3žÞ'>¿æ"1l"Ž?"bèyóÙNAGNbll3FGL J1411.4-0724NVSS J141133-072252?잠dJ9%?°"up®P?€¡|`?vè¢IM¿·?¹	½~ªÞ?¯N«ðËÓJ?í
Tq¸³?¯4e?"žœ?'l†èdzz?–SÓÞ9+ˆ?³::¸
å…?©‹å­
?íóä–÷K?šõh¼¾½?ˆ"v¶¾*?w'`#7?´ôpuƒ?˜dÕ؇›?挢KUÖÐ?¤ìaÃ;Ð?´¥Éˆ¸?šAòD1¯z?Ëz'IdH¸?¥J¢ˆëS4FGL J1411.8+5249¿æ§ù ñDÚ@N!uŽ!–SÀ:ÎÜيJqÀ<ÐÒE²'¸@mòGۋ×@'åp1Á?¹ù⯍ 応Oò†qã?â¸îÞðeÙ@
©3)ƒ?ïZTª|?ì¿ä¢ŸÒ˜¾¨¿ÞíC÷Ò¿è~bÁ–7å¿Ì¸éÖrèÖ¿Úa€Îq"AGNbll3FGL J1412.0+5249SBS 1410+530?ï°U
Áv"?|ôƒ˜E'Ó?HàLuQû[?AÇèò×Àf?'\·ÈM;f?{ݕ¡1?>?ï ý"»ë?"â¥yŒÂ??³~8·îp?PqÀ7ð5'?†ÂþßVn?"77¼o?îÀ+Ðt¢?‹Ê¼Å]qâ?pI´)ÝÐ?kùmÒ]P?¡ôsƒ}?‰ù.Д"?ï°6nâ¢?l¦ãYÈ?Qã.˜o?Cíùg‰30?Ò.'á"Z?k‡ßè?ÍK4FGL J1412.0+3836¿ïù,F7¥@Qg¸d"À;†2´ˆ2À<Ž#â]@ ˆÂ%ÔÐÒ?û´{'G–?ÉgöHòL?½ËPËÊnN?öÄçûý<@ì$+#¿ïÿìêy…þ?ïùàÌ^¿Ö ³Ô®C¿Úf÷~0ˆ¿×>?©c;¿èr'~túÿAGNbcuFIRST J141208.2+383521?ïPD+m?±<žûä¹?8nõ\GïŠ?6Fš``?••Â¥!=?±<^¿õ/?ï«V[û÷?…gÆnŠ¹2?CœgW"îr?VPcpg÷?ƒð²sˆ³G?ƒí.åC2N?îZD¶Ñì?"‰¨[þ'ø?f—S1¹Å?d¨Žû3U?¨òHòßŔ?"ÝIè‰?ïQ­E!ò?wƹë«ô)?bßÇ7ô²ú?T'€é¬xw?"n^tÃ'3?vœ­Ãd,4FGL J1412.1+7427¿íj['Ôþl@DÆ	VÀÖõÀ:¢!óoÏÀ<£èì¾Ü@}s±¨"@‰Ÿ
vá?ºüg>ÀZ?˜Ð—e?}w?Þx~a.ï@­{£ºZ?ÚÙéëÁ"š¿ç E…EO¿âªÜí¬@e¿àyÊÇ9¿èŸú¦ú«,¿Øx' Ï-zAGNbllGB6 J1411+7424?ïGxêzÀ=?˜Ùªç*O?pÕ2+«Xa?i7$'¤?'Û–%½";?–-"£úŽ?ïQKO©?Yk«>Y?Rö=J÷÷?[·¤JÉÀT?"µv¦û.Z?‹³—+	eÜ?qkp^?|#èÉs?s×A²fÉ6?aÄFÉc‰ô?¥l²ü!
?‹&™ÌÙ?î£êt®ˆ^?"Š¯Ä2?"Ó?Ͳ Ê?k]užÖ¨? ŒˆÁªñì?ƒÈ☃š'4FGL J1412.9+5018?îŒ}~}Uä@OHƒýP"À:õênžCMÀ<²Àsøö!@ê²:O\4@SÌÐþŠµ?蛢Íu¿]Ô³tV×?˜¥w¦Þ.R@	J«GA1¿¦À"üêæ¿èh'Zà÷&¿åBl"4X¿è…y¼"€-¿éKV?§¶¿ïÿ[•R<AGNbcuSDSS J141302.28+501927.4?ïï[—Ä·?iÌÿ4¡DU?Aý]S¹œì?C³¹'B?XJ!ÎÅN?fŸ]¡²þj?羚y›…‹?"€K|—˜w?@•ûšs›?QîêŽ?…JșdõÕ?ƒ…X>ä
?îþ£M4?†·Æ(9j?lŽ…gÃ7¬?`F– ·K!?œ™Å¡aÃ?…·L™"jØ?ïÏ/ŠHöô?`çû¤6?[gÏû&V?Iû¹ó]T¨?qŽFܺð?]'ö_É«4FGL J1413.1-6519¿îu=HØÀiØá®aÀ9»1'À8jÀ;'™,ŒP@ۓÜ@]=@ý"$½N«?¼2sÓÝ?™æÇþ9‰í?à.ßFL¬@V†PÀb¿îæÉbµþ?ï"2¼ë®9¿ãbà՘Mi¿á™óÇ™k¿æ)'@¶©¿â"¬Ø:¿AGNsey3FGL J1413.2-6518Circinus galaxy?æ¡Õ'ü<?ÀD=K£Œ×?†Iæo?€'ÄÆAT?ÒÃ`×Ì×?ÀZ¤C?å€vëO?ǹ¤ZÁUý?WÌerÞ?oo)0º ü?ÔçEÃÂâŒ?ǕlópÚJ?áÀ+õS	µ?¶Fn‹KÔÇ?¤Bø+Qh?Œ¼z?»x?Ùü¶T'h?´Ç.xTAÏ?é²BmJ6?¤PÏ!Å??•§OÇ>êç?Øg©"?ÈèLýbùÍ?£dáTE½È4FGL J1415.5+4830¿ïÑDô¯G‰@O~Ü~ñxÀ9¦tÿ†À<K'5!Iý@Á½CÚu?þDv×ͱÏ?¯z4ú]©©?©ÎЁ6ï?ú#ÝTÚLè@Âƒó•¿åMðMÛU¿à"œÚ–¹ë¿Ýý±¼P'á¿Ýš¿]οà™xa"·¿Þòky˞AGNbll3FGL J1415.2+4832RX J1415.5+4830?ïøca¹Gt?Dy®Jœ'ì?3å®ø¿Ë?'t7ÕÈ-?K+üeÿ?C.~ÿçæ?ï±Ä[N ?'öÖ41O?7›dtæ™?I‰ë
äO˜?'Ò…G³?'bE´ì(?ïAgëSî ?zp']åL{?dê±[o>p?Y‹ìŽ—?•5¬jT/?xC=XÜ9?ïè"'žû8?Sê#K7ž?){›ÑDÎ?B}Ó¦ý³?fF£ôSL?S`')|4FGL J1415.9-1002¿°9©üG¡›@GǤô^À;Ep÷¹àaÀ<Ù¤?åÉ@ÿ0,#@SPÊï?׿-BÖ¿?ïÿþBe«+@"ÚųÔ@¿?Æi†¿ãÍÍlê?Ѻ(»
,ª¿æÁ|^¿ïþaßîé?Üè=)T¿ï^-ôAGNfsrq3FGL J1415.0-1001PKS B1412-096?îÐjò—ì?«q×Û5Ç?œMhŒÂl?©Ò±`0`?ƒJsL@€=?Š/ˆç¢îy?éœØBM´Z?Ç«Ó "Bˆ?¸W7'5Ÿ®?Áýý]žÂÿ?ºÂk\½|?´—ÓqVï?êwT¢K.?¤$¿Õ«L??±%Nà2»X?›Q"ВýŠ?» 
sԎ?œ2Te±G?ìF–c;Ð?µ6Ú»ÐÃ?¯zö4Iîã?²õy=f¹?¬£šBT/?£'/hO4FGL J1416.1+1320¿ä±ó²ê£w@PyÛ
Ø0À9ÈÔ¨c`øÀ<X¼ˆ±êÉ@*ËâA(>@*ÈE~R?·h_ºÐ í?Áq}ÝÑØ@¹Ç¼Â"Ž@
{NÀWs"?îB # –x¿ãñãr*¿Ç¿äQ…¦ž¿çÕj*@Ej¿ã×MŸ7¿ðAGNbcu3FGL J1416.0+1325PKS B1413+135?ïÅóðº‰?rFÌÓZ2?Ys9±ô[?WušÊgrø?v©9\úÓ?m˜™¸Öœ(?ïT ›Ãõ?''þ4'?`G¹Àå?nÔÏ¢Òi?"bõO€ ›?Ê@ãRv?ï³ñŽAs?€ßˆ~ÍàK?q=$?dR(1†ÃL?˜†2Œ·È–?~†"aT?îá!–ýÛW?'K슮·)?‹ºÍ¦Yþ?t
Пppï?•þfM@h6?{Pv$Á&4FGL J1416.1-2417?ï\R6ÆY@ATïܜM©À:—#	¼AÀ<e¤m í@ ÑD€bï?ûI
Öק?ÃpÁÂ؂?Ãî•ç2@&º «q@
	œºá<ñ?çžX°›=ß¿ïýf],+?ïæ¥á{…‡¿Ô¯–[ ¸¿á·¾þX
-¿áåàš	+AGNbll3FGL J1416.1-2417NVSS J141612-241812?îUH™â?¼qïåL¯¥?€F5–òÿ?Ž)eòußF?ªé™ò0¥-?ºÓTÇà¯?ï~F8ÖË'? '|
Äé?P•2d1?dÑç†J‡
?Žlÿ#ûIª?ŽD¬ßÏì®?í""Í\‹f?¥þñ®ñ?g6'V¸À'?c:9-êÑ?¶1¥'eÞÖ?¤øpn¢f?ù˜Ý"?©	£æ‹?g…$;·E?d5=æNø?¢õø.lH?Ž×´"æ‰4FGL J1417.9+4613?Úàï-†÷@P§Ú¤ü¤À:ö¤}"jŽÀ<£QùÇכ@^"JÊÿm@ç#? )?ÆhŠ'¾Ú¿ž"$\"7/?є¨½õo@¬Y=ÞÝÆ?ï¿á—_,¶¿å¶XKñp¿ëÐ÷Ÿnd¿ëñõáõS¿ïìu߀-¸¿ïè(‰ŒAGNfsrq4C +46.29?ïó¸/H{w?[~½~t»?CÝ
ŸzW?AþY&ÍXÌ?NeÐr«/?XIïànÆå?ïi#xÊÕ?'áÿÌÛ±?V/ɱ|àÙ?kÔ¼ìoÑ%?'y¾õÎ×b?'%mŸ'˜k?î½"ôs}'?‰ƒEñ1?t,úc=?hÂ{_ÞFŸ?¡¬ë{Í:?‡î«|þf®?ï›Âk¶?sù~CU?xë¦!B?k
fRþ?zÔ¤ý‡?g3a­4FGL J1417.9+2543¿äÖUÜ_¼@Q¦W>«6zÀ:l–ç7²À<N1©Æ7‡@"Ô˄£=\?õ˜¡Ú°»?Àh3›
-?½âËfÆ2ª@9f1A@Ä3D{-¿î3ᱶF¿ïµ>ì¤Ù?ïÿë""i·¿Éçã(®ÊÙ¿Ár$	ʄ¿» !6ö%AGNbll3FGL J1417.8+25401E 1415.6+2557?ïddÙ¤"?"ö钫|s?SòŠªo"-?Qa›û׳Ø?'4< ÖT$?"xѳà5ˆ?îÓ҃Òed?¨l«öš
D?e"eõ|Á?p¡7φ?¡r|zQý?§§«€/ï?ìOe‰"?¡÷ÿ
P?{FÄRÁŠÆ?k™¨.ºjb?»Ðeª—š°?¡±–Ýëî¼?è8ÎĀµŒ?²ï?5À?{2"yI!?xØ
?œáÉ?ÎC0J_Œ?±è|±ªo.4FGL J1418.4-0233¿åã­C£@JÓÙý6÷äÀ8>Ùtzü À;Q‹Ï¬{@Ë¿º?ú<¯c/zA?¤Ê"0'o?´€$þg#¦@Äpë$¦¨@ÓAaRü?ç¾¹ä"¿Ý=ëì:¿×_nû`^¿Ðqal+¢E¿ßÀÒÆӿáO	ß3ØAGNbll3FGL J1418.4-0233NVSS J141826-023336?ïÔGfwCe?xa•¢?GÑJ6^`?d9¾Å" H?røR›'?›IAº0&b?ïBª?¶_?–1!knÙµ?[#Ðûùèe?dp‡*zÄT?•øzùU™?•p]@f?îÔ¢]óÊí?Ø¾à¥hü?€PˆÅn`æ?>6·Xë?CoÞÏr?5"¥)N?íµ2ÈbpÐ? ®X×#^:?sQºœ·¼?cÈN?±!N!	? ã@f54FGL J1418.4+3543?í¶ö )@QfY_í¦aÀ8'cxu\£À;À®ã­¹â@á¨0¶+@ Á['—?Ÿ¸ådHT?°ídášÓð@ÙÂ~•1@fTȯ1?Ô"g^¿àEí οâøòÔô¹¿àŸ¼ÞÃp¿ã¿''Œ6¿é¨¸á2ŠlAGNBCU3FGL J1418.5+354387GB 141615.9+355650?ïéá"GO]?`Ñ­§ån?=wi®è‰?7œEhv?bo~'Ó S?^nôW²ú?ï °ŸX=w?‡DU´	@?IZªx/UÄ?]BZ#W>×?†>-'m¬ë?…•»(U?ï>X!¥A?†¬æűe?t©¥€"×?uoSz0?"
'aý?'N"úUoú?ïûv5
ér?6(y-¤Q0?
Ò=¾f'?HJHŽ+?@¦N°~P?5®pñ$%>4FGL J1418.7-3504¿Ûwô®=?§@8xW£UÀ9õ\ŠD'À<+!xö‹ã@qªqX1ð@.…Nˆú?Ã;™‰(ˆ4?Ëz$‰LD@Iæ?@0kؖ/?ãaýKÙÆ¿æšáBO°Â¿ê]3ímVE¿êšn«¯EÓ¿ï VíLŸ¿ï÷6ÍòfºAGNfsrqPKS 1415-349?ï'ld6?'ÆHB,oú?Š4´|qaÙ?…€À A›?‹ðGêÂ?ˆŽï4¶ˆ?í"^1+?®þÙf…+?•Ä\;|Tã?ŸÑ-"ê´9?«Ý¬nÂ×?¤!ë%Ñ?í¤‡wÓ"Ü?š¢›®^D—?–²7UÎðž?ˆ]0.'kú?ª^l×æYü?'ݦËÖ?ìâ&,¢Ú?"#û?0ÌÓ?§šûÌä¥?ŠbŠrü¸?ªÅ<8íÁ?‰‰,íð{å4FGL J1418.9+7731¿æ˜ŠL8–@CI›Oe™À:^§Å¬GÀ<u¹&&Û6@ fhê¥%?÷ªˆºNE?½ÊèF$ý?Én#Ê	£î@aNÏq@Ñãá'Tý?î!ƒ†Üþ¿Ô?Íà?dÅù1§¿Ì%œq».¿à:aÙ¿àÅþ¢ûrAGNbll3FGL J1418.9+77311RXS J141901.8+773229?î†@Ö&c›?2JD‰æ?—6J齋I?ŽuÐÌýƒ"?˜šQvZ?"&~̨¾?ï
¨¯Ü€Ô?›'á¼'ç?j$·Äö¼Â?wçõ'1=?›fSÑ
¾?˜ÿ±=y~?í9So? MfðnH? Ë¼ûh…?•0F— '?«£ýÒöõŠ?"
EêÚ0?ì‰èž—À?ì;¥ûñÃ?Š¬AE™?xŽ˜S¢D?¸m‰êÙ9S?.;Á€˜4FGL J1419.3+0444¿Öa|$qW@M«=ÈK^À:¹Ïþ°t§À<†ËÈ1]@ ‹ÆGLš¸?ûÑÁ(SÜ?Ñi‹ T?Âxš$W"?ôÈoU"qD?öh\૦â¿ïû9\B 6?ûª0¿ãA؉B	¿×­eL`¿²lTg
{.¿ïü-þ@`AGNbll3FGL J1419.5+04492MASS J14192748+0445138?ïBVêÊ=D?ìᔣ|¦?Xcá×å'?ZH9£î+í?–.ä‰G‰%?CibbY?ï–°ˆÛÏ?›À³¤Íó?g'4|ªä?vçþ]¬?œ<ã_RА?˜ê°û#?í})¤‰ýr?•?~ñ5ŠY?ß›T"=#?xjJ,¶À1?±Ú¿qŒÍ?"ýXáó?ì.8ʛ¡.?ž,_èty?RfgrQ?…m€¹º$?ºìo^V=?›hZU¼·á4FGL J1419.4-0838¿é_Þ§73j@H-¬îàóËÀ8o‰u_'®À;§™Ûøó@7ë@Iݙ£«?¢XšËÈÀÏ?´':,v«ƒ@?-É@ÒûO—¿ÑµPx…x¿áOY"J¿â¥j­¥j¿äš÷g«
¿æק¼r¶¿ë‡4<G®ëAGNfsrq3FGL J1419.5-0836NVSS J141922-083830?ï¤Àû}6e?€²¡µ›Ðè?Ki²€ïR?FpBX¸¬þ?…%ø£qÀ?€ ¥
ºÄ?ï~˜£sÛI?‰1gUŽ?NîÉfÔ2ð?[KRÏN>`?ŽjꌛêË?ˆJ9¨Æœ?ï5Þ÷¡a?‡óºÉZ=?výÉ‰Ø?wŧÝ|­ù?"ˆ(®©?'
;$íÅ?ïã:¸Xa?Y*¢¼="?7ktôOÏe?,Ñp=ø0?i×Ù	ô?WÎýi†R4FGL J1419.5+3821?çÇï
—ç@QfÙ×À9×À¥wnÀ<=®ä"yw@ùÁ3£'@"ª¼×ŒC?·‰êá¦?ªA… ,I¤?ð\Kv @
ÓìÆè1W?ê<C²\´¿Üœ?¼-˜?¿çßáa¯G¿çç×_w߶¿ç9ö X:)¿âzŠ&_AGNfsrq3FGL J1419.8+3819B3 1417+385?ïÌpN¯¯3?n9<ŸCS?T-Òdxä­?FIÒH7Â?t¼d
-?k¸b1¹Xf?ï—"k1?‰?ÎúÒre?IQ×XW#o?WuNפD?ˆ§AˆŸÁp?‡Ó%™˜¼'?î÷Dâ˜ä#?…3™+#?s‰ƒo|?d€408O?œVMŸŸ?'¶"{÷ã?ïX¥s'Éz?w·HÄFvº?´Ÿ"½€?l}à3å›r?ˆ"‡!ò?q¨Ò'«Ê4FGL J1419.6-5153¿æmÚµ(ý@!Iz»ˆÀ9W"Iô?ØÀ;¨e­ÙÂ@	$ÕøD @§£Àd¾?·<TÄþLL?´4ƒjX8{?öƨü
,8?ô¢=õƒû"?ÉZB×%+¿âŒ*°­²U¿æ;Þ}yR¿æ~T>p©
¿ç,åÁX¨¿ðAGNbcu3FGL J1419.1-5156PMN J1419-5155?äÖ~ϊ³¸?Ãt¾U?'(óËV?‰ðýs"Û?Õ@y‡ë[Ú?Ã]Òsïøí?Íd~~õ‹¯?Å͊|>ÞÐ?ʑ§D0?ÅòäÈ#Ž?âxöq'?Éס¡xç?ãÆuȶîÄ?¯!C¢n5¤?¬.\É3ðØ?'²Ùùxڍ?ÔíHÕk¤[?¬Ô?ï Ù¥?Öm/¼é¨5?®G§G}ä?ÍÎ|ÓtÀ?ªHéžIžK?Ú«'Ù\Hë?¯ö‡+÷Õ4FGL J1419.8+5423¿ã¦Ë[ç!@M&É[ÿWÀ8íL§xnÀ<MäHêT@v"Ž¾@¿–Aö?¢K†¢W>'? –:iˆYÖ?ù×Ì%Ýà@F˜T _¿µ
[b ¿ãÔ ©Óy¿å4°
õ'¿äØuâÛ,¿è!gßjr¿å¿eÁ$øÞAGNbll3FGL J1419.9+5425OQ 530?ï±hOÅ?è¨3 ?G4;µk?Eª_ _†?'4«ûx¼þ?}Þ¯Léuý?ï‹ïVôhé?ŠäJ`/y?Kßå D÷?[ïžàù?‹F+ðჲ?‰s+‹("?ï5¾·Ü?,ÂNüh?hÝ
š?[™…AA?–8íb؜?€=+]‡n?ïõ›`µ©?Eû	rV?@C¬o¡k?4
m¢0[N?INï|ìK?@¶ÂŸÎ4FGL J1420.3+0612?íÉÛ<•÷<@N!	á*QãÀ:š¢Ûa»À<^{Ñ1¶[@9÷8Ü"@®"ø?¼'¡Æ3+¿²Ê'+'u?õ7u'c/@ñ.ÖØ?ïô˜ú7¿à×Nó[¿ëâËf›@¿Þ[*4ï ¿ã«ØáX&¿Ýº¹9r•AGNbllSDSS J142013.69+061428.6?ïÒ}@û{û?l}‡‹Çà?U©¨~*?O©ö	y³2?q]õ"x?h+÷{J	r?ï"j8Çîü?‰¿Ï!Ÿ\?J0q¨É?cýñtºtf?‰Bj³'¯G?‡"–"TºL?îÞ)¢?‹;|A±Ò?k†ÿõç?Z'Ðüƒ? eýnÄÇÄ?‰®³=ns¶?ïdIà9ãá?zjTæ{©3?t|¥§4'…?dÇøwt¼¡?Œ¯5ì¾e?uªUBqE4FGL J1420.9-7920?èûˆñÀ186†¥À9ÍCÿ3QfÀ<Ќtíé@	6rWá=@±›îÞp?¾Ï8
û?ºRýRü|=?ýs՟Ú%{@Ñ
è èÃ?﫲~lí?ÈJw]¼"¿æ8ÿûÎB¿æÖT5{¿éˆݬ!¿ïûVƒšTAGNbcu3FGL J1421.8-7920PMN J1421-7920?í…u!ÔGË?©×næ'ëÌ?Žmz³…C?L¾ä6Y?°§šíF?§Ǿûaù?ë?Ÿ$?¡¡ÛÄZ^?yXÝN`?…håàrÌÍ? Ù5¢BÀ?žQ^ $Ö?ë*Mȶā?¦ËùWaá*? )Ï3A•I?R.BÛɗ?¾˜ª ©R?¢·ÊðäÕ ?ëô›'!ð?˜Ú6=®·æ?­mø"I?'Ø™Å/ª?±Ìlz®y?Ž³ú±¼ÉØ4FGL J1421.1-4614¿ÅßÅ;Í¥T@+¹¼ýKð™À9ü]¦¤DÀ<
rÎ\@®ú²Ž22@ÑÕùµ?º´Fn#t?É	ËÛ¶µ@Aü#Òm@^06Ô}¿à'$,Û¿ÔiËá'n¿ãÕ2ÌÛæ¿ç›xqοïX(ñÿŒ¿ïÿ*¸:n'AGNbcu3FGL J1420.9-4615SUMSS J142047-461431?ᜫ»G?ÁgԊÛW¾?ÁäÖ"Â6Z?¶o-;0JÚ?ÓÔ=Í(UÖ?Àؙop‹±?êCp'éIÂ?½Âs8üwá?ªh2?ë@R?¬{-ìê7à?ÀX1d`ß?¶ìªŸ,Ü?æ
,o.™¡?¯@¯\æ*%?½… ^ÈÙ?¡êƒ»ð|?ÉÁ35?¦·—<Z¦?è5«o‹¤e?£sûëÛ@ù?´ê'Šé'?˜''Vœ?Ä´üÎù£?UCN<F4FGL J1421.1-1120¿çr{[–@Fæä:§›»À9ç"UUÀ<>¨È
Æ-@"/¥	9@;û"?¼a؍bÇ?À	WC¡ë@ÿ|í'hs@
¡©7ò4»?ãS¤¢Œ1|¿Þ*߈'4¿äåZ—ü
¨¿äH!ÂG³¿è¾ó…ô¡¿ïêñ°±äAGNbcu3FGL J1421.0-1122PMN J1420-1118?îîÅ[ø'?"3z¹ˆŽe?t±ø´•?p¬ƒï†zþ?œû'ÐÎ=?'|¨"ÐÜ?ïÚÐT&?–lûÝs?edÆͽ?p@\>â	?š'™\¡…"?"\%T¥9Ê?îþ.	JŒñ?….?²mR?toÍx5°r?hÔo›{ÿö?›Kx õ³?'$fÃ?íøˆªÈ?‰ØV…¼o?•ùO£ˆ2m?w7À±ÌÔ?¥'߬Ñ:K?"Öyû;‰4FGL J1421.1+3859¿ÕCٌVm©@P÷27Š°ÉÀ;‹õl(GÀ<_±´B'L@Smfò'?ð´V´A¼?àœBUåå£?ïü{±QFD?øÞÅ7­w@	(ïÀAÏ?ì[Åޜ*¿î·¾b¦¾E¿ÅZè	ã¿êÎ`ÐU¿ïð&¾°ªW¿ïýÚ rfOAGNfsrqTXS 1419+391?íwJKâ?»éC·'¾?gnóIÜo?rV''5¼u?³Š8+X-v?»†mƒ¼I?í—.^¢Õ?¸î"üHVd?'ïwx&º?¤Ìp¤Íí'?­^YÇž?³‰cs–*?êƒÎÔؚ?¥‡C¹2nª?¥ÈW¯aù?"݁yͪ?ÀÒØÔR?¢Õ|ñ?ëdj¾tÒ?¸üÂS­'¥?fjSáC¸ë?møqâ\?«¶ªyÖ?¸ú͏˜=²4FGL J1421.6-4819¿çÀjŸ—E¾@'Àì1"À:…ñ7`ÆÀ;öp5ó@A- Í›@fQó蚉?Õ½1ø?⑀üâ5@	«f/ßÁœ@‹\¿ô?ï«ÝhüBܿ݉EcŒl_¿êˆÂÔ&¿é²3ž½ð¼¿ïÿøsCÄ{¿ÓÝ¥q"AGNbcuPMN J1421-4820?íô3|´¸?§I-¦"‰º?§Dö:åe=?£Ì%ÎçZ¢?'ï³zžž}?'ÞªÕÁ±?܁:òMt?ͪáQö¶ò?Ôq¶°t«?Ìh'‡¸;ö?Îh®–{Á?Äío2ò!?æ–·'‡?®‹=
,µ?º‡'v¸?¡K¡Åÿ¦ñ?DZÜʵ?¤ú'v
)Ï?Ð»È \®¨?¯qûœ‰?Ù®GqW¡?»?ÁÀ|ãÃ?ՕðO1ù·?º®o§—èô4FGL J1422.3+3223¿ïýCŸ^vû@Qh~AN~éÀ9t‡Ù}µ8À<n±lôõá@zæ'Ì@ù©™èt?©úg\'¹?§‰ÎÒ`‹?ùzà…v@·½WÓ|?ïÿù³>†¿ã€!ùO¿æXÞW(Ü¿èwhð?ï¿Úgéek•¿èg˜_ݶ)AGNfsrq3FGL J1422.4+3227OQ 334?ï¯ñìʂ?'ÕK/²Ÿ?1Ž}ˆåK?<‹fwà X?ƒw†7-?'ó¨îÝr?ï°Ò|ž*?…TLnô?AP]úŽ`?R ~ï'¿?'¶`¶¸ÌÚ?"9;Sê?î]€Ašì?œ¸N¢Š52?kôÅþ/tn?`£½§R?¨o;œYî?œ{!héÀc?ïýIùß̅?,p§'vø?	ׄ© Ð?¡ôHƄÓ?2u@lg¶¿?+Tb'Bq4FGL J1422.6+5801?Ð÷«a†ò@K›<Ž%ÈÀ:ސ†Ë`¼À<˜Wk àJ@ Ü}78P~?ö$‰íT+Ñ?ÄÂ'ϨŸ?γõ:,Ü@
›Háa«@I×áRëµ?ÓT^¦ÿ^¿ï'ᐩ0?åôB'KÇ¿¬‹Ü"à¿×éû[Ök¿Þ²'#ƒ'ÇAGNbll3FGL J1422.8+58011ES 1421+582?ëÓ‡Q3:?¹š¥]î=n?£8µ"Æ?¡"ì_"?·ËqA,ƒ$?³öH#èƒ,?î‡"~è?¥FwàB"Ð?qCIªªîo?|¯ÝY©rÿ?¥fJ¡b³·?£"}…¨'
?ëÃ|Û"ú?¢ê!À!®?¢ÑšÍO°I?"ÿ›OŸ?¸{KÀc€?œ.ÂyP!?ë¤Ì]Ò<Û?ªt=»±Ôw?"' hˆJ?~@F¯E 8?À#¥®°"?ª\ÂÒô4FGL J1422.6+8150?îÂGd²K@AL\1Y>À;¹$Øý\¸À=\-þ@@©¤æ©Â²?õ'
0Ûj?á4ڂ˜?è•Ú\ØH+@»7^;º?ðuR½g¿ïÿb`ÈAÎ?ïÿ|Ìy?'ëËRÔ¿àÏ8·×rB¿èqgù
¿ïÿþBe«+AGNbcuWN B1426.4+8205?ïhÌÁæ×?•0â6Ö
?x'|öÎÔ?'$iç
,£?‰íK'
âþ?øÈ[-?èׇüΧ}?Åùü'|MÚ?»¼Â!±'×?Á=<PN¢º?½†ý÷Ù1=?´cTt@>?êñ~zßñ?¦<€Ž*?§z˜.ñ?–%rñSn?¼ºŸõ‡ñ?¢)©Î?èúj\(?²ô« °?´h­%É?°-¶0xPC?Å[ÁÉ*Ø?«I0˽_4FGL J1423.1+3738¿Íù2dñŸ@Q#_€™À:îؐOÀ<JãÁÛØ@ýÔö¼à?þ׶»%?·«u#I?€¸!Df@	ŠC»@Ò÷BOù?àã;z)'¿Ûþ\;ë¿ÞÀgmÍ¿ÝR•äƒLÑ¿é_6&,ºs¿áš3½œ®!AGNbll1FGL J1422.7+3743NVSS J142304+373729?ïɹª©¼?v"´àJN?eijvc?fÇÕ}÷V2?pn¨uæúD?mp²8iÿð?ï´
à=ã0?'CS­Ÿî?DÝÛ	Ï&?UtižÂ"?»j֗L?€ð¥Ôqs?îÊP<?ŠÁ,HÚ°R?'í&Ô?~y°k?T(Uª?ƒ»Ë¢•k?ïÝ¥lo?l?[¿·'?:—Bäê·?,G¢1yre?o«Nôµ?Y÷{Ï`ƒÓ4FGL J1423.5+4524¿ä;UcLÎ@P'û?¦ßÀ;>eV›îÀ<å'ê)Ôæ@§$íË#@‡±¥)Õ?Äßʇù¿–$ƒºVŸì?Óâ:\È-@K>ôŒÚ?ïÍ8ÝŠ¿ãà'ód¿æ	ˆt®'Æ¿ÙóÿÁ–¹¿ç-ß×kŒ@¿Ódƒ7W…"AGNbcu87GB 142138.0+453705?îù¶ß{?–@¶¼F?\Z2|LJÂ?QܘJš%¶?Ÿ™<R÷î?•Ô ÷g¤8?ï`«0œ}?ŠøR+[C2?NÂü"Æ?Wû1¯èÆ?'ô‰´'·?‰úžÂ¬:w?íên®Ö…¯?"7y¼""5?w³¯´†ø­?caOÍü.?®bŸÅó?'ÿ8ðãÂÚ?ïÜs—ÿ‹?€SŸN?|ˆH¸¼?d(h4´Œ?˜ˆ-à~?Á0'çÒ4FGL J1423.5-7829?îÁûç'ÓÀ0x,äd™À:ŸSÌ/îÛÀ<,ƒ2O¥@ö€»|Bq@8xñÝ(?ÇŃ»5÷?ÓscúÑAü@	ÂsBûÅ@Úâ9E›ì?Áùß?>¬¿ä¶Ñü·v¿æ[`Fþ¿ãMf H	"¿ïÿôÕ÷?íx= ™AGNfsrq3FGL J1422.8-7828PKS 1418-782?ï•1¾‰hè?ƒ¾ŒkñéN?r4ï4ˆ¯?s ùG=Ow?™Ãan2?}p¡ã=?ïµ:Üí0?Ÿ2è‡cš:?mh!*Ë?~«Ýá^0?™üTt0T"?›p¢OŠ³ç?ëïê[Ú?¢XKQUÚW?¦Là]l`w?"z]c$çè?µZ<ørÿ?šìï1šBº?îkÊ
8
&?'†¹§29?s˜zt)Ÿ?f£B¦óh?¦áìM0Øj?}9 'R4FGL J1424.1-1750?âûWî9À&@CÜÛ7ɚéÀ:³Ú°À<ixX×1«@ œ­çYk?ý&Á½¥?ÃÙjM%Î?¶¥"Ÿù@Y?ô™6Òúä7@
ŒŒ÷¿ïÿ;ÒDÜ?ïüé)ú¥M¿ÛßÚ¾[¿ÞÄÑ ñý‰¿ØI3$Ň3¿á>—jjAGNbll3FGL J1424.3-1753NVSS J142412-175010?ïï7¡t~?Y€ 1W»?&'Ð*ĝ? ¦'"´¾Ì?^¾c^ž-?X‹tybv£?ï¾è)?€@â63¤»?;Ï^®n?P\Œï1œä?~ۓu‰–¥?~§W×N2æ?îíŽÚÍí3?"g4_"èÌ?dY~D$O†?Q+#ë³®?ŸÂôݽϴ?ƒozR•ï ?ïœÏž"¦?lg~ž#ƒ?Oßýä0Û?@Ÿ©bF7B?†Î™R?l
|‡üè4FGL J1424.1+2917?ìË9sX6@Q`ô^NÀ;ólàÓêÎÀ=|ñÃ&[@!mÇÏâÖÏ?úA×:äØ\?Óò۟x€Å?¿ÿ°ÏÁí?ë)À°3å@œÑOŒÊ?仪›I¿ïûÕÎÔ
?ï+Îð"{r¿Ï<ÑW "_¿ä.Äf¿Õ
5ã盅AGNbcuNVSS J142408+291800?¨b€?‡…@—ƒhN?D‰‡E©u]?AÂ^.ETa?ŠJ}sÈì?‡Db?îõ
aQ?¨ûë´ÅQ?d›½ÙT-?z1T²%?žÉh#‰C³?§ç"J¤?íÇ…Ø ÏÝ?•;¿¼6?räÁ0°v?gnd¥oŠå?°•…+øf"?"Y~Æo"X?îžOºWN?'ò Á€Î?g#" Ç~m?fAâËòš?¤¨Ë ƒSJ?'kxiA:ý4FGL J1424.2+0433?íq€'Æø‰@M3•1ã¨À9ÚÃvõØÀ<(9oV•@Xlþ†c?ÿ®Gx?¶[²Ù0³Q?ÃLßV½&@4±?¨Œ|@­¡kõò?ïGŠ¾4ƒ•¿ØÓØDO:P¿á3§—‰!¿á'­"ãY׿æå>³™õà¿ïÿôw5ÁƒAGNbll3FGL J1424.3+0434TXS 1421+048?ïõÖś!?JŝpþBÛ?>«óÀ;ˆ?9r—jâ?IQ‡	[N?AÀøà·?áü~?…ûÉY­#s?Dú¹Ø€?VF¹ÑÓ¯é?…Å[ã_œ?"ìzQ¤ k?îõBÏ*õf?ˆÌGcah?'‰=ÇÀ‹€?~ßEöÀúÐ?˜6Á
j?~6"_~Õ?ïÇ6A—µû?e€ÑâîM?PV–?@N	±=Å?xc]lO][?c¾tC…'¾4FGL J1424.6+1447¿Ã'ŠŸb0@PBçÀn¹À:iȉq-jÀ<uÑá߃‰@äk*Í^@7ÆZÂÄ5?¾G\5
"ï?"Æ4=…'È?ח-ä>ÙZ@
ô(Ü¿æ˜\þ2ËY¿äžOv_Ø®¿åÃƓͨ¿ÜTF=Ñò¦¿æÄ¢t´³¿Ý/"—Ú|¹AGNbllSDSS J142436.29+144910.5?ïßU4€	?cçnÚ[ƒÂ?9@§ª}[?/âd¦\?m'¶Š§?
?béÆïæë¼?ï¾?•Ò
b?·>vń?>¿Zbzc?S1Ì¿mpg?~ô?vó'b?€«|¤ÜT?ïA®þL{?|
.ê';‡?czz{Ëw?Oör/?•ZîÄw+?z&žÎƒ?ïÆÐäÄ=?bÍ7¦î?JÅèbªU?6©Ârœ¥?yVtàåÇ?akG͖±4FGL J1424.8-6808¿ì§Øä³yÀ]{ý§`,À8ÉBÇ$íÀ;€нV@Yà¶Bó@ç>?Ö¯¥?«ç"w³?Ì._6qV@%€Ãÿ@:Š*»À`?ïõáμ'¿ÝU|o?¿æ	àž»Âc¿é#™7t¿ç|}Ê0:Z¿ïÿ/¨;ôAGNbcu3FGL J1424.6-6807PKS 1420-679?íó@ôŽÓ?ªCÄ:¶qi?•àvw/ˆ?Ÿ†‡é
g¢?¥Ûµ{7µ?¡¿uþ¹$r?ä6¡¹'N?ÎðxÃx
Õ?ªf¬ÿ#°?³ôïÕ͍?ÔEç
»†?Ì1|ݱåc?éCÿÈø?®@1Lx.?¼k) ÿÚG?¨ÿ ID¸Ù?»Š¶f‰Ýù?¡³4£‹õ?å{'ÄU—²?®@îg†™4?·ae·"Dx? Ñoì‰M?Îaß~þ?¨®ÁÃ(A¯4FGL J1425.0+3615?é°äÂóì2@Qn'"šVÀ9؏AQ(À<
v{‡`@ SEµöâ?û€ û?¶ØÐç
À³?À,2ñÅ«@YQûuVÄ@TxžÍ5'¿ìâT1?î#Cœ7̿ʸÂ~À$¿×`½,à¿à±Šâ¾w¿ßIà>¿jAGNbll3FGL J1424.9+3615FBQS J142455.5+361536?ï0_8ZÅA?ŒÛGÂ`Š?‡%´§–õ?ƒED,¡`z?ŒÂ}A·º?€¹§^ü?î5DD}®L?¬Œx&ƒg?AÛzÜG?šrák›†1?¤ŠÍú¶÷"?£"?f\?ìtrˆ	Aü?Ÿ«¨¨õ¨ ?™>V5‡NÄ?@C¶Ü?¶Ö2To?™ÝáãBÖ?èIÜSH?§îçýoP1?µ9¿Ëc£Þ?ŸjRC§¸K?Ä?©	?¤,·úý4FGL J1425.4-0119?í¤
}ºô@JÒYÀe¶=À;lœù	À<ÇÏï–ü0@!à*w¢Ï?ö¡›Lø?ف9ÜÆÑ?ߎ0Ú¾R@ŸL{ٕ2@ˆžìää?ïû°&äp¿ïÿùëñ?ïþ¹ä'¼0?li|Š.¿æm›¿8º‡¿ßõ b‹AGNbll2QZ J142526.2-011826?ïm‹Pš»?—§cœ×ñ?TP•ure?RµË5-?'	Œ•WG?—E²V$ù±?îÙÃØC"û?£Ù;¿'?nxv&?ì?sÈmÛ¸? |;f\O?¡íuçIYÏ?ëóW

ˆ¿?¦8{8?'@ûÐý?r¹äêÕ?¾$§GŒ?ì?¥ÙuÕ¼†C?î,õ#*?šèjMÛÝÆ?mÛ>ÖeÆÓ?j°ûMq%"?«Rû i0ñ?š>à-'³"4FGL J1426.1+3403?àðo&±ù@Q!灃ùÀ:Kñq…À<˜Y¸Øú@zã ùµ@ÓÅåQÿ?»æþ§:l
?¹
Ùͼ5ü?þBu
n@Jzpßf-¿ì
þ‹¶­¿Ö6j?Žá/¿âYÍ "¯Ó¿à™_æÌR¿ã/\äÝdË¿æ@U$õ'ÎAGNbll3FGL J1426.2+3402RGB J1426+340?ïÀ2Hù²ý?ptH'ÛÞt?T2› )ûû?I+°÷«ö$?zÚ4›´?n`J7xú?ïè@©»?‹àè('1?Vz(?c©Ç‰ñà?Œ¶'?‰"·ó.Z?îÕ ø'
?" è­Aµ)?q.b1Èd.?`žï®? €$7VQý?'¾õÅ:¨'?ï©iÀ;:?|÷iiWñ?ƒl@ÿŽ?nÖaõ3"?"²H1X"?vŠnš¼¹*4FGL J1426.4+3625?å[¡TµB@PõöM½ùÀ:Tغ@ÙÀ<F<"¸@/fRÅIÌ@A'Ã'ë?¿
SO³F"?—'(6êÎ?Öˈü@›©×Te2¿âìËð¦¿å:"yÄçü¿ép÷б^¿åË¢Ëq'ú¿á­òKâV¢¿ïÿÀéz-AGNfsrqB2 1424+36?ï·†úDä?w™ ÞÞ&?fÛ6šð¯²?_€©N¬t?y	¡5e6Û?s×.µMÄ?ï'c"y'x?‡xê{Ĉ?J‰·õ!•?\¦©s·q"?‰¾›âd6?†#—rÂ1?íã>½šëV?'Ýk?B?"Ÿ(ɟZ|?r'4ÿôxš?¬¤Ióésò?.åð¡Äƒ?ï|m¬Êƒ!?v¹Ÿœ£?qyÐqÆ?bRòôtíK?ˆ`†vÿ?rãn¿ã4FGL J1427.0+2348¿Ö
Áœdr@Q
´·,À6Ô{Ås<8À:º¿&¼@` ãzcH?ûHcF uÁ?Žec~võÍ?­ÃŒ #$â@37ÿJÎZ@Á¿}ƒä¿¼Fa
a"¿Ñ˂Iñ»š¿Úú¼#\Q¿Ø"a`î{¿ÞïҋR¯¿ÞÖ-¾ÕlAGNBLL3FGL J1427.0+2347PKS 1424+240?ïtYô]kð?ŠÙÀ;¿£Ó?EÙôôÝKo?F|¹%1ý´?ÅñÌ«—'?Š9ñބj?îë°v'aG?¤Êh²¯§?qÃÿa¡>±?¹Snáº?žñb«‡r?£Ì">$£?ìÞ3	nÛ?§¥D¯—^›?'?¸‡K©?Œ(½²š?´¾y'Ȧ>?¥õÒLŸÏ?îC`SP'k?6ãä\»?qïÊ°-4¢?g]>ù49?©ŒtñB²?t–
['C4FGL J1427.4-1823?îã\)€@Co`|A™þÀ:_'‰±ÅÀ<YðHÒש@ l)lŠî?ý&ÆÞOâ?Âɋ9Y'î?·õºgš?öVuÂú»ó@žé€â"‰¿Òº|þƒS1¿ì¿"zM£ø?«p=]a7±¿ävH@áqŸ¿ºÝå_&s¿è1D±	ø§AGNbcuNVSS J142726-182303?îú `}/|?"Î
P2Ÿñ?b¾JFïo¼?ZÐnj
¬§?žT*§|"‡?"*Qs–Ö)?ïK_äuï5?–ö¡ãå?Q}‹a±Æ?Y"®ßp·?•{+˜‹þY?–X"'ðGI?í,?à[Í?—Ò(éA?ø—›½?reKŒxm?´|ì1©ö?•CeæÈ?í¨58·^?–‡ézì½è?mË®žµÃN?bJ+"pK?±Ïù±D–ù?–Lçœ	Bô4FGL J1427.6-3305?˜¢«4MnÜ@9–r§½HËÀ8ŇB_ À;Ȓ%1ñ@B†Òeh@–'³ÌJÇ?¥C8cõ?¾"yNõ†@¡aä÷f@SÅm2¿Õ©ma­D¿Ö¹ã»üšñ¿äe0Áhë|¿ærᏥ¿ål¦â,…o¿æ\_©÷AGNbll3FGL J1427.6-3305PKS 1424-328?ïÍ=‹y?Éh±ôÒ?`VP̏å"?s<f¼$ïu?"w)½y(?}?S&¥?<8?†"
'@u?R7ÐI¾š#?bVî!xu_?‹	6ö:)n?"÷<ÑäÎÿ?îhùÑfÙ?˜
(O¿?‰Ý˜µ?¼?†P+îh´¿?£Ê5™Ñî?"[,k$Ê?ïªmd–²?n$/ÿâ‡?[¾ÁµN
?G7'~+?'Lp0' ?l*քô'4FGL J1427.7-3215?ÚªãU¯@:X_9K{)À:-70îµUÀ<C¯æâøˆ@¢Éübç@ѽaõ¾^?¹ô%j‰?pGڊ$±?·­=+H@å?›\'?ɛj^˜'¿èO¯'Âe¿âPmk=e¼¿âT§BÔ¿ãÌ'áE¼¿ÈÚ*~…AGNbll3FGL J1427.8-3215NVSS J142750-321515?ï°0t÷ü?¬êíP­x?OâR¸5~ƒ?zŒ§Ne?õ½–œ(ý?©±"ê*>?ïÇná•ýF?{ò`Ã~?0ÿõ^"ªÜ?A1ÊIgÛ?{8ß"…?yÞÑ=c/ª?ïŒKô?'äք;r˜?f‡ŽWU.	?T®4¢¾j¬?œ"ÒòØ?À`3¤ÿ?ï™`)Qx5?n±«=·öf?KÁZH/¼¬?8T
ŸÁí?‡ëà÷?n²—´qš4FGL J1427.9-4206?á š(4Ò@1DûC؜åÀ5µ¥BDH.À:'¨æ=·@áÃ;Ôl~@Å,?#+~?}P>à$=X?¶­ÿ7¿E@1tÿ†]}@#ÐÜÑқ¿Áã¸á2Š¿ÝÍ+—]7¿ã¢U_­å¿âÿÀ?Ѐ¿ç¡¢4¿¿ê¤0+@öjAGNFSRQ3FGL J1427.9-4206PKS 1424-41?sbÃÇ?¡ÊÞzê?a	–çÔý?bfIš¢?¥eŸ[V'»? ®çp?ìyÉIE½Ï?Å·|¯…"j?«@2¢ø'¾?ÀJnm2_u?­#8È«ûb?ºiÕvÈ©?ì·JR±'?ªŽP'7)¶?šÐš:kR?",ºÉ­I?³ßé[ò?¦"\6¢"?î¼5l–Ð?¡Œh
Äó¥?×рzâµ?"îbL踉?Ÿi»Ï´v?œ"Õ(ò²Á4FGL J1428.1+1629?ïö³_µ¿Œ@PMØ/×^ À:EçjÝÄÀ<UŠ"C"@ŽZ"Zî
@‡ëy`>.?½?s³VB?½ËÓþo\.?ûöÚ7›@§EaE•?îäӉp#¿æ2-¿€Þã¿å¾Tdc¿êß !s¿ê}'gv0ß¿ðAGNbcu3FGL J1427.2+1610MG1 J142813+1629?ïØ*A<W?{A6lœlÅ?Vw}/·?i·†fA?lt·>?p?#sý"?î÷³ÌÿQˆ?Éóiý•D?sͧ¾'ý?ì˜…Ζ£?œA¶&.6?˜1ô`Î?!áÌ#?‹n¼vüw?yZ®ø¼¦?qé\p T?¡{(â¦@?ˆw2M?íûÐs
<§?"pØ|_d?£ÕIv"*1?'£4$È?˜Û^±0–?€è@PþDÞ4FGL J1428.3+5635?Ïo—§üÞ¸@Këæ`ɊÀ;rrä#+À<€ß×@ϔ*ÄϨ@Mv«Xÿ?Ñj;<ìðY?ÃãC]©~?ò†	êdH@Pÿߞ¶¿ë¦ %9um¿Î›C踿ålZÁ'œ¿æ£ßÙj¿ïÿb%>Ô?ètÛߏG0AGNfsrq87GB 142651.1+564919?ï…g–m<?2gÆ»ì?b¶û¬7¼?aò›âËo?‰ø['_£1?»&Cv?ï5úz‰;P?˜¥ë͞á
?Zàu¾óV?l»½"Åj`?—'©R?–äë 5Ò?î$xÐNO?'¤r¢òa?+ž$ê?s_1€ÏÕÉ?©U+;w'å?¢œ¤¢(??ﶾšÞ…P?mkhڇ?\·Š‡­?K£ÙçÈ»?}Ÿ"®lq?j7Ûÿ°Zâ4FGL J1428.5+4240¿àOšSöÃ@P9©¨–hÀ9t"à4êÀ;ÿO†Pº@!¥ÿƒƒX?ù°³â;ë?«6ý[ú–x?•'ßÿë™R?í?jCj¸Û@f;¥¿é1•Ùñx~?èR€f­¿Óù
'åÍû¿ÙL;l茿ÊÓ¤—Ïj¿Êß"$m¹AGNbll3FGL J1428.5+4240H 1426+428?ïÇR,?±ò™V7/?XÒÐÏ&\í?k."h?œù豨'?±0ñߞ_'?ï™tùë»?ˆ¹A‡4?FÎ.ªô#¯?T³U
3k¨?ˆ5ÞϕÏS?‡¢OïòË?í¸°÷·?—ÔÄø^t?vëÛ,?kçÛ÷Åì
?°×‹ºw?–§£PöD?î>]G3Kœ?ϖ¼Ù&?x'…Á"?fןßQQ?©ÚÔ¦ö\?Ž–D¸Œ`4FGL J1428.7-1017?堄gáÄ3@Fà:S¸ä¸À;I|­ÐˆCÀ<œFÙÙ$Ê@#
‡þZä?öõbÓ3ï?ӗ…"P??ÑI¬|]I?úèââ¸Ç\@þÁFÆ8¿ïÿT_™?ÝN=»!~«?6Ã
¬?ÜZ'±m˵¿àn¹ª?¾ëƞE·AGNbcu1RXS J142844.4-101801?ïiLV°?¢Á4âF?WÜP°{ҝ?Qr¦äö?…ª"äÙá?€‡™Ý_¡?ïgˆU@?"âl;¾¥·?XE=—úµ ?nßeÎt'é?'Šœ;Ýìƒ?'œ"c'?íeUtU ~?™Ïá¢ü6?"W­nVÑ?yZñÎAÆë?²J^»å1@?—(¡Þ]?î@Ÿ"ÛÄ?œ)°!ɛ?oiCK—{?iíãô_)y?©ÿr}ŠNM?›Üøv¡â4FGL J1428.8+7429?Áº²ðúöÎ@D'À~áÀ;s֑q­À<ÿž)\ñ@!}@¢‡~å?þË׿o8?½Ӑ¶¿¶s"ölƒa?ú{x| @	#pš…?ïâ½—¥¤¿¨nâXFµ¿æwÂ,ém¿â°â`‡Õ¿âd ()ö?"cþ	äAGNbcuRX J1428.4+7429?ï®±°wÚ?'qwó¾?PU×1MQƒ?\j.ßøò?'t˜­¸_'?3/+]?ïY<©at9?'JœKžÿ0?V[þÙ~±?f]m຋Á?"r¹Sãàö?Ä¡yY*#?î;¢',é´?•Û<äéN+?jÑ);ÖA?oŠ£"{ò?ª˜Êû­§S?•
Ð٧Ő?îL¥ämXœ?™¢tüR8?|}¼ø":æ?uNÄÚFf?§¥êîÞ?š‹á¬Ûy4FGL J1428.9+5406¿Ï¾mt³ÂK@LÑM"‰aÀ:¾VCæÀ<Ÿñpv‹@ЉÒ|97@èÃm¨z?Ço<8j¦?¿ƒb¯È°?ôOÆl`{@¶¥ÇzS¿Î~¨<¿3¿êm-]0]¿âP÷†®¿ì¹›Aº_¿ÝäYüu±Þ¿ïÿ-r)HAGNfsrqS4 1427+543?ï®:Ý\·'?ŠQ÷p¹qÄ?R¢ÕZõÐp?O–'&Ò¸š?'íýseŠ?‰qýŒ	Õä?ï"4Êÿ\?‹Åî–s+‹?I¥‰£ûØ?[([%Åþê?XtïéC?Šåôе?î¸EK"K6?ˆÃÃN;?p¤¯°c
?dfǟÔC
?¢gQ®èì?‡CUá.t3?痢Å'?n;}`œ5?X›+'eæ?J›F
ÿÓx?ƒ(Td:î°?mÿEDšÕ4FGL J1429.8-3058?ï͍eiøR@;Voç¨mÀ;&Ìÿ!³¯À<'ütðm@ ´1ð'ú™?ÿ¬ÇÔ?ˆ?ÌZ.õ‹ÝÄ?ªŸFàAÒ;?äþraFl?þ(V†?u?ï]}>o&~?ìl]¡Eà_¿èç£è§ô¦¿ØUÃ`½Z¿ì¦€‡ÏÃ?ßOµIùHVAGNbcuNVSS J142940-310013?îi<Ó´Ü?£?t{ÓƼ?kYMÞRy?d
ûê¼Â©?§¶ªTã?¢Ø"Õ´úÄ?îM¡ÛÃT?¥uq= _?~钾RÕç?…ù›dFb?§RSŠyoý?¢®q¶Ëì
?ìˤN(L?œÝî[ÜÐ?ŒÌö#Ž|?™¡Ï•?¶	>ÊOkÎ?™ró)9z!?êúёª3?¤FŠ›nŽ?¥Ó†;Ý?™­)<—"?½?ì/'ÏÚ?¢Úڙ öÀ4FGL J1431.1-3120?ïÿ6tŽÐÆ@:ßlœ
"À9ÛÖ¶Zš€À</OC427@òˆQ¬y?þ̦6`^?¹"y™I?³¼f"HÕ1?ûº"ԗœ@-îdÍ	?ïÇ P ¿æçÌÍ£Œb¿ÑíÔñhŽ¿àŸß|&í¿Ý¡l å}É¿Üå6%+ÁAGNbllPKS 1428-311?ïúƒ²÷g7??å·WŸ½/?éÝ)f!ú?µ·â®R½?C3ø}6e?=o¾,·?ïظ‹ˆD?|Qʋß+°?:?z퍏N?R‰¦¬]ä"?{¬cu?z'A|Ë[Î?ï–FoɈ?ƒK-­å³z?h"sâ¡îE?`±W¨¤Ø‰?šœ¨µ²'?úÁNŽ?ï²1¯®?k#õS¬í‡?D–êMß|Q?4Yï¾Mߪ?'*%"¶ƒÍ?jCåÜS÷4FGL J1432.2+5051¿ï`Ù²õqm@MÄ}¡ìNrÀ;Œ¡c'wÀ<ÓGºÇè@âõLÈ°ˆ@Ú6º§0[?Á³±]Z¤?Šo*%sÇ?ÈÔÁÔiy@
qŽ¯/Øá¿ëÿ˒:)Ç¿ßii:¬#_¿å÷·ÒiſݑÅÚ뛿é"±œ]™¿×œªZ±ý>AGNbcuNVSS J143217+505603?ïÏA	Î?u[ú§ü·®?PäEœ8ª?HõZ@˜ÿR?t_ç
J?s^ålÞ)\?ïœYEäË3?‡lŠ:S^&?@I'_ì?RjLU!á?‡åeG4j?†I@ŠþÔ?îî\îb?ˆƒ8¨bóQ?l¢]rp‹z?bX#âLG^?ž›ˆ³ñBP?†Ñ""à™ö?ﶪy!îÁ?j…š(?TÔõ.Pº?CÙ£šl9?u†#t™?jBÅÖ>ài4FGL J1432.8+7648¿ëÏu!{a@Co8q`•lÀ:ôÞü*ˆÀ<Äh-ƒ@
Ž+§M·@Œð=ë?ÀA°¹ñ¨Ï¿±¸©)Y•ž?ðôu£KÜ?øS¸8ìË?Òpõ5¡¢}¿ä‡£'¦ô¿åJù"–,þ¿æ°ÔéÑÀR¿ÍÇNH7|C¿ïûܟ¨§TAGNbcuGALEXASC J143211.35+764355.6?ïSüÝ¥Ÿ?–")#h2?€Š…†x"?yx°ÆŠ¸?•Ð=¡Š?'ô܈dƒ?î$¢Tÿ;?©K߶Ã?zdRÀž]?Emù[?ªiPWïXm?¦œëˆ?í fè?"!àR4ª?Š¡3¤'Q?}P+‰Ã]?¯QR&ä?<ªõI}?ìú·šÝ¡?›Tƒ‡(x?—C™%¹W¯?v뒋#?²_ùº½?˜)xÒ/S:4FGL J1433.0-1801?ÊTU¤™ŸE@CIM½øôsÀ::DZ°èÀ<~ó%&*@u2¹e¼È@(ãúü?ÂÆñÁxÛ´?Õ}BuñI@	'^VÍl/@ù
ÒÁÙ?×Ýê¬\¿Ó(ؼD>s¿éS³`À	E¿êR·ÈXÉÆ¿èÕÙ ð¥ð¿ïÿì»"AGNfsrqPKS 1430-178?îóÿ#»_§?¨>~Œô‹?‡mH ð)N?"6
8œ•?•Éwxöt?¥Ã€|ý®ª?ïyl)?'C¤h
"?V«,r÷cõ?m|݇é?Žä¿k ‰J?f¬«·c?éYÊ¡Ã!Â?¬Ý&%•
±?´kì"×p1?¡†æJF9?Àbß6‡Àß?¥2¸=\
"?ï€9‡s?sjõ'͆ý?dŸ¾=V?Ü?Rí	­;õ?ŠÉ®°$ÓL?qWr®\á4FGL J1433.7-7304¿è*1Q†°^À'`†`ÔÀ;°¥R4€:À<Ï0é¬×@#1©kž´Œ?ڐþ?‹†1?ãќ	¶b'?ïù½€Ô{Ã@®ì?þÛ3,}6?ëå² ùõ¥¿îޜ¾H'¿ïԋÝï4?ïŒv›gÏó¿Ç{ô'žUk¿Ï¡&Á4éAGNbcu1RXS J143343.2-730433?èï«;;!?Çž
lþ? Ù'=E?Ð5°šHö?ÊgF9ïCg?ƤNÄÍou?àÚq{5I?Ò|›é®ž?Ðð2o?¥ !æî?ÝMTˆö?ÒŠÑèN?êIhú‡o?©NńGm?—yÐx#õï?†ûwNq?Ãë"c€?¦ËIã¡;§?äNCœF¨.?ÄàlHÿë?xGI#õ0'?Uož›…K?×[¢âÚâ?Å"¸™H4FGL J1434.2+4204?îWø—€å™@PC¿rq7À:GÞ
ò}À<¡("V@éùK/ÿ@—!œ1ú?¶ÍàsØ(?‹¨Mˆì?ш¾ÀoœE@_ˆü"d¿áÀç@Áf<¿æÉì}l<i¿æS.°ís6¿ãFñ÷(Àé¿ê''ÿNTL¿ïÿÉ¿&FAGNfsrq3FGL J1434.1+4203B3 1432+422?ïÎ>'jŸ¶?sî8X7p?`KÁm»R?Y…ËãҍÎ?p»"!Gš?pÊ໼?ï–	i¥w?Š5}»Œ?PÜ%(ÑÄ?c7%ò·R?ˆb¼ ñ‡ù?‡¦
ä2ó?îô72ýÓÕ?‡Š°Œ¶ ?sÒHÏÌã?j$ì9»ký?œ"‡lRL'?"…Ð#c?ï¤ó·	¡[?p-FNI?w>s
<ݳ?eáSZm?vG±mòsÒ?cE(øLs4FGL J1434.7+1950¿é´.Eì&@PR2LƒfQÀ8· ·›`À;¯–ú'è}@ْÔ-"8@)(v>K?£ß¾þQþ?ÁŒšBç±@´[זT@Â*­¨š>¿Å²@Äì-»¿ßÃp,¸Å¯¿äì|•|Ôg¿å1" Ü.¿è`½¨"¿ë‹q¾‰=AGNfsrq3FGL J1434.6+1951OQ 253?ïvÛC_¨ä?‡µ¥,Bé'?lZuDރ?kÿ®Þxì?‹2'ÖÞ&a?"9¦	F¯ ?ïf
&m?' &˓?W;¤ËW?aìÂÐ],?'ÍéÄuÔ?'(âDe?îý£ü=?'Ð&Ý·n?‹`íÕuÓ?ˆŠÒ¯®e?š7ԕ½…?Š"zÂ_E?ït¤dëv-?}8ç
/òp?jãÖœ–ñ?]+
FA
p?Œñ@»O
?zӖH 4FGL J1434.8+6640?Ì1ùöZ†@G°K±¯:À;1ñÛzºÀ<äŸê²ð@!gŠS*Ÿf?ù~N"ÈQ=?ÄMoßáÒm?½£Ž¡)A(?ù`¿'țæ@=qá¿ï'ëk¿é,%Â!ù?ïý7cCœ7¿Îëð¾ïi…¿ÞšÜDŽû0¿Ðï¯OäCâAGNbll3FGL J1434.6+66401RXS J143442.0+664031?ï½$èqÍ?z£ÑR?DöàZ،?I†ä´áÇÁ?~Ï/»¾è?y¼»,g^a?ï)rþ"#?œºÊþ³¥?Yá©Kp¼U?l	Ôÿ«Ž?™>÷"¯Ó?›9¥¡,ä?îZ§ûÙ´?MôKÌ×?pû17rÅ?`†èÏd:ñ?«êïYT!t?‹‹¦Ö4€?î®pÝ£l?‹åFŒW?l²ì´2C?f¦p[Òð;?£Xöýü?Š¶xZx3#4FGL J1435.3+7120?в
õ6Ã@E¼®§GØÀ<*¡/"À=˜w:Ê@:ë&ÿô?ÿ ´%6n?Ö¬æ0x?æH"Lx~—@~*šÞ=8@:¾÷!4¿ïÿúÁҝÇ?ð¿×V'þõ¾Þ¿á(ۋ¬q
¿ïþš9҉¥¿¡NöºKAGNbcuNVSS J143518+711818?ì'c Ô­(?¹dÙJ¾¤¡?¶6ÝýÕ
Û?·UE¡Ñ?"ø#î/…?–h‡WªWI?éqÅw`?ÀÙçhfðö?µ5g¨>Ãñ?´EtIK t?¿Bb,;¤?¸âˆoö?ævÖDºmš?®™L™!g·?Á«<t²Éã?¨œ(/Sñ?Äyjxc·?¤Ëõ®Ø?ë£AU6×o?¥F1>½·?»rCŠl
?£•gÁÙ¦c?ÏˆJûb?‹t¬ê_Ë4FGL J1435.5+2021¿è̽öù¤¥@PRžì¿±[À:"F}'ÒÖÀ<]	ÆR_@!S«Èp?ÿ0L齞\?Ìã^ÊÙ?Ïqßy¹Õ@hÞ£Žåá@—Ò- ¿ï]ÔA5Tv?ïݤ@;¯Y¿æV>@¢Â¿ÈðšÝ;"æ¿è;`gÊ¿ðAGNbll3FGL J1435.2+2023TXS 1433+205?î%Ã~Â-?¢åzñü—?'†ãÍÁÞ­?ŒE©''X?¤àV8²íÖ?G´vNª?íߤþA¿3?°'MÇ"=Þ?"Jš˜äð?¡æܶ!Ï?§½ŠÎ—š^?¥œ0–¯q?è"Ýø!Éæ?®&D•Æ7§?°ˆÜtx)ê?Rö, NÐ?Ålå<Ãn?¥Ï÷@ÈU?çR¼ï]'ç?©/?yÕ?ºûVÕ"*?¥­²¨#ô?Å7`×ø¸M?¢üô<Ø
4FGL J1435.7+6148¿ïËÔužÎÉ@I›ÝÁç–}À;Ÿ{DDÀ<ì'ódK@ÌšY²ú@t` Ò?Ç;XE¼LÍ¿«F&CÐS.?âå7ýO@ª)¤"…?ïéóïP…T¿æxcôœ¯¿éwÙ.Úß¿·ÅC–'¹¿ã}:ÞxEâ¿ïê¶øO1–AGNbcu2MASS J14363365+6149514?ï¦G…l¾?SMPÐ?a…ö;½Ý?_g~{¯,?'&½'o ä?}½5""N?ïYœL›?'ÙY,)iB?PŠí¸XÁà?]·'ôœUl?"×Mðà—?æ¥zwÝ?íÖÜ÷ y‹?"Íå1Ã?€ãº3?tÆÀÿ…É?®Y?ßs•?'ßíÒ}?ïK¦z?'½!¾Y'?q?65Ù,?ftÇ"LÙR?'M°mG$?€¤¯bÌ·4FGL J1435.9-8348¿Ûƒó]7òÀ5ˆx·¡Â]À9ñ¸'ƒ$ãÀ</R1%;ú@™]f¤S@ë=Ñææ?¼ÄŸ½Ü*I?¶ª›I?øSëõ‡:@,'y@³¤¿Ö.á_+¿æÁIÁ•?¿è½0w—¿âÎý'¿ïö6¾.®¿ïüɟpÉAGNbcuPMN J1433-8340?ïô}S\QM?LmÚv?:À¤?Ǎ?29/Y¤'?PU0@
sq?GVò'·?ïËS»DjQ?":ŽÉ?0·b%Ç?E7 ªœ<?yJ°×¨{?}½Çy?ïS)%žk?yÂ/Ho<?n"‡Zr?eQ²	§?'Ê=8
t?tšÇà½cˆ?ï›Ç9øÅÈ?oÅ6:Ê:ñ?`Ñg²ªýÌ?MùP[A"Å?"Ùו#ι?m¼'ðR4FGL J1436.9+2321¿—ßcqLE@Py©?)
»À:y|ßýÀ<Q'N"¢Â@ý1Äs7@‰
5
(?¾)j1¢ˆ?¯ç¸Ëôœ?ëSÛIgR@Ño‹þüJ¿æCŸu¦ ¿ãdc1Ù¿ä}P·
H¿é›K_ú¼t¿Ý'ù\wпïîÊM–ŒAGNfsrq3FGL J1436.8+2322PKS B1434+235?ï.€A(6?'Í`?fXAØ&?k†jÿ)~9?—lŒÒ¾;.?'d¼ñ˜µ?ï‹Ì ÜÜ?Š+–ä?Kƒ¿»Üý?ZÊ	&RI?‹T»ÿJù?ˆ»_©)ÅÉ?îÓÊá,7?ŽÈvÞâE?x—CýÆ?hž˜ai¹?¤ÐimŒa?‹¥@¥á55?ïJÑåQÍ4?|ú[²ò
6?væé€i5¤?fv"ÙÁr?ìõ¬<?y,'Æ
%4FGL J1436.9+5638¿î.öF²…¾@KuâlvÀ9½Ö»cýÀ<\u¼D¿M@†òÍ<‰H?þ©GŒ†Œ?®¶cC‹	?è'u¹?ã#×?íUÙ@	äùÄQ©?íö–•[$¿äEmþ
\z¿ß1uBø";¿Ú›[慱¿Þöú2`¥\¿ÕVÄ-ÁÚAGNbll3FGL J1436.8+5639RBS 1409?ïã"Þ»ø?_¼å	j'?3Lb¶hÉ?&‡p®õ¦?js• vï?^%ÿήÐÚ?ïšäY ?‡
˜."`?F²ß÷wª?V…ÑxÞ3?‡ÛÍj''â?…¶–žƒ=?ï*
ærØ?}âT¨$x$?e9ëÚ¢I'?Yq­ßV#?˜¶P³µ?{¼@¨"4f?ï6žôÁé?~x—|o?qzŸœ52I?[®Æå†eÃ?"Íy€µµ?{R$M)Ú4FGL J1438.0-3128?ÂW=ØÂh4@:!¦'¶(FÀ:Á"‰cÀ<[¾¤ž@Ö'-ŒÚ@9ö›Ó/½?ЁôRLÔ?֖ê<Ê5Ä@våÚºÌ@	µŽª}AŸ?ﯭ7OË¿Ùùð'Íó¿ç"ré+¨¿æfS¼?¶Ï¿ïç'JïŽ4ÁRÆ!AGNfsrqPKS 1435-311?î<úŬÝ\?ª2Üü[HŒ?xC)ÿŸ?}…©uª`?©'ñÀÊD?§NGÞÑ?îSXm¢'?¤R붃Ú?"[°ºïÎf?"^GËÜÀ?¥³Œ÷ü
?>\©{ú?ìgÙt,? "Ýö3À? ÒÞ{[è?‹;pûÁ˜u?´^ïE ñ˜?˜¹4€'–?ì™Ðù#9?•É"°ö?›Aƒ~(M?'[ebªBã?´a7ÖÜ*?"þA†Õ84FGL J1438.5-4207¿îÝ|a>M1@0w>Õ'åÀ;g˜ûÀ<'œ£9UŒ@ ÷Öå¼]?þYÖÖ;
˜?Í0!ÌX‰?²Êö†M?äâ6kw@z7y>s?îØàkæ(¿ín¯½µƒ¿È¡šïÚîοÝÓÙ{±Ò ¿ãÉ?2Ȫ¿Ø;vBýU¬AGNbcu3FGL J1438.6-4209SUMSS J143836-420705?îyx
\T?‡>ïôÀê?S'Bü§ô#?IeBÕSŠX?§ÏEtû8?%Éí2?ëܑÝ[»Œ?¾íÅ_ʬ?[&LJž"?†j_rCB?¾ðK˜ÏÔ?¾T#ò¸Zÿ?í|Çjú?"ËÙm¨u?w$Ç׎Œx?e ãQwm?²§x1_?"Î&‰
/p?è`d;"=?¨óx̅–?ˆ~E®·¯>?x¿›æJyì?ÌöŠ¹4?¨xã²"4FGL J1438.6+1205?á"
rZ÷"@N\UÀü´òÀ;jœ×;»˜À<Âk"ÿ@ XÙéëÁ…?ÿª¼¡Ü^:?Ðj"2¯Ö?¤PŸªª¸ü?Õî$5inY@@šÒª?ëæoÖQ°Í¿ãg¾Šêª-¿åØl¨ŸÆÚ¿ÝÊ2ÿÚ
¿âëî›S­ý¿Ë¶^Ì>1"AGNbllRX J1438.3+1204?ïÌò¼?•bœ¼k|x?ZÍR"'Ñ
?Qè¸`Vx?9Œf]?"ÕïÂæ€O?DœÆý? ×"À€Œ_?jFA3}!w?t°WCÕx°?¢s7¢û½ÿ?Ÿ~™…·ŒF?íÿú,ÕV?'ÆÔÇ.°Ã?tê³CBÕÌ?a-éàeÄA?­c֊OÊ? ÿ*A?íeï¼–
?—´%qIÅ?TÔÃLá?sŒî!Äý?²¥ìÉ»F?–Ò!d9ú4FGL J1438.9+3710?æγS¡_-@PO6&,ºÀ9+Š¿â¿À<3"l;'@λ³tâ@zŠûq%?§0¹[Uç?»¨w­áz.@q|å-ì¢@AÇn.? ©r]H81¿á¤¢š¿æNS™Û¿ä¿-½R†`¿ëö{A"ÊÓ¿ïÿþˆ0»ŠAGNfsrq3FGL J1438.7+3710B2 1436+37B?ï´Bõd£?@/=뾘?eú°m$?`´ØmÎÂæ?zá-?w¼'?z"±Eé4µ?å°Â…?Œqæü¢?OY€ùE¥'?]Ì&n–CS?Œ.";h?‹1|VæՈ?î¨=U䞞?'«±½â?ˆ
`½iNÅ?·ö"º?žó$䷄ì?‹FԟLlò?ïçôkH?R‹Ù5¶ì´?Q';6é@Î?BÅ{²®&?`4íùwˆ?Lî³04FGL J1439.3+3932?î°7…äl@PêÈ`V'À9åßÁœ"À<cv­‡@ú—Ý+ê•?ÿ<ÛØÙJŠ?±ÍFšC7¸?"'¬¨{E?áªSÆP±É@¸ï&&?ï"ÞnµÀ¿àç­=»Lr¿Û×!ºdë¿áKs›Ù¿Ú|[Wð¿å§«ÅìAGNbll3FGL J1439.2+3931PG 1437+398?ïÖ§‰ÿS?h1$…îÞ??EêÏ=?:8µ§ìlª?r÷~9}"?fä!È`?ï¢rÉö;˜?†¡qϦ…?D2fÈôÌß?SÀólì?† 'áÍ2?…on"¶Ãz?îûKàð«Œ?…€½h¿¤Ÿ?jcè$Èa½?]i²ÈVn?JÝQ'??ƒÖ[Âà!?ïTs1ô8?v°^ˆH?u°«…Ë-š?a™´7‹F?nà
-¬?s•üª1ŸÐ4FGL J1439.5-2525?Ë#•Ñü­@?ZäâmHÀ;VìÔªÀ<"1í¸ÕŸ@!¡[YíÝ?ùˆ²¡)±?Ð<`CÃX?ÊH)åV±h?ü‰l«$™?÷˜ùöüv3?áÕT%B|?ït§!A™(?Ìóä餿Í=þhPK¿ÖagäjÎ*¿ã9oÀtzAGNbcuNVSS J143934-252458?íuÍó¦÷?¨ƒ×ëUk?'k—'‡Ü?|¿ó+Ԍ¨?²p~´¾?§s"'
¤?î˜<Œ€Ð? ôðRÔÀ?y#ˆ6Xe–?ƒ=	Z@‹?£WÆ13.?œ³.;Ç8¶?í7S>+‰"?™5Ô³Œ?Š#}F_Û?¢cù~º?³öe×ÐÎ?•	
<ͽ?ê}Ì
?¨ßüXJ?žmè匩L?'>±'	?Â>.}:±?§DF:q4FGL J1439.7+4958?ïÇÅàä¾@M–ýuâlÀ9±vi騦À<~[òoÅ@ó@7'´z@0«~žk?¯ey"øõÂ?¦&ŒÝ9¬?öa	ÐcZB@¨öæ%ä?ïôÁrüvß¿ã±b]Ã)¶¿åªbÆ[¿åÕò—Ÿï¿ÝnÊ£|ÇQ¿ïÿ–]ÏéãAGNbll3FGL J1440.1+4955GB6 J1439+4958?ïèþ.) ?]TjÁi?6/G'1ú?/¸ø¥C"I?d;èõͪÍ?[L\Õ{2f?ï™ÇêoÙ?…ª@?Hˆ"S7Ãg?X€`þõ'Î?ˆ/"À0«?ƒ¯$@IŠb?ï3ëÖtp?|¦(—Š<I?lx ͹ƒI?Z*½²Ê|¡?–žkzA?y"kàǾ"?ïÃm˜ÄL_?f՟ªÔ<§?kƽ"i?]›nºåO.?pf'?ø?[y<iÖ"4FGL J1439.9-3953¿áýƒø·P(@2_ûz_A¯À:WKtr˜¤À<Eˆt®'Æ@ ¯ÔH@ïÏÃøõ?ºB3@Êž¿ ±ÇÈªÿ?箨—›@ûÐE}8?ïþ*"y¿¼WÆåW¿éiæM§RÀ¿ÓýãÆ
–¿áWpßçÞ¿Ü -1'r"AGNbll3FGL J1440.0-39551RXS J143949.8-395524?ï;‰£•ä?ž¥þÉ?Yä"fUQ–?]èýu?–ðƒFÞ'?*vLŽ
?ï•^£G·~?ˆCé§ÍXb?EIZ¡§Ky?W£x³KÉ?‰SÁƒ÷«Ë?†¶·/€OÞ?Ìÿ'(?ŽbŽ§Ï'?rÈ0'QT‡?fÜ5"¡—?¥œ}+ÂË?Œ†€—Hë¿?î&R0Ü¡R?ˆG
Û!aÞ?€…"Pn5?f¨¨y¯=?©"{!ÏO?‡w;ôw4FGL J1440.0-2343?îµP <²@@elaR*oÀ:!…óÊg˜À<OþR€ÖT@vq·þ4@†ý»'"?¶÷*nh"g¿œ[¶ùÀ–?å®:ÀÆ.M@´t'ˆÛÜ?ïõi~sÎY¿éF
¹üæ¿á?ž¡cê¿ÙBÔ{lÝÏ¿ä¯ÄH™ÌÅ¿š"!J'–AGNbllPMN J1439-2341?ïЫ.rÌE?j!"TÙ@?Fm6If>?=Y­"Të'?tÚ{аÒ?h­8G¾—?ï©°"hÞ?ƒ·iÀ²Ñ!?@»I£âî?P|&`s'?"³]'§¾?'«'`iîù?îÝ¥ÙþÈP?‡3‹J(#?hÿ‰}gð?TQRýLýá? ¤'g{¤r?†*ãéK?ïó׳}
?|@ï2ÀÕh?srh?ª"?Zy…
E¨"?˜Äêù¥Ù?zt¡ª½4FGL J1440.0-1530?Ĩ!&–AË@CïìÃã?À9"卍óÀ;ß>>)0{@œ%"¤DÃ@½´'l¤?µ ªDŒ¡ä?–è>€¡Ú?ä&áìÂ@@beOåñ?ïöÒYԇ¬¿ä³5è³2¿åŽF´ð75¿ãkã]²ã˜¿Ýg5c'¿åò#žj¹²AGNbll3FGL J1440.2-1538PKS 1437-153?ï䫦=•?pK´˜E½?7údß)õ?3;é/[»"?hU
0ð†Ô?nî|"?ﻆ[?òº?"™â)Þ?7þУ8?H¾q-á'?€f19~5:?€X<!Xú?îÁǔöP/?Œè‡'1ò?s%_áfæI?féN%â0?¡~Ú´n U?Š]›p±fg?•'¿?t*ü"Ï1¥?NqO=rß?;ï/e™D?Š5EÂ?QŠ?s´­¿x€4FGL J1440.6-3846?£Û
ãZ'O@3S™åóíÀ9›Ò<xVSÀ;ýF[.$@!ˆjüx6?úËP`j£ã?¶>iN?S?¨H‡-[X?óÏ
D& ~@P7~òNg?ïÿîBt!¿è•Óa'¿à—«öÐ+¿Ï 	cr–¿Ö;'}E¥ü¿ÐŸ[DÊ4lAGNbll3FGL J1440.4-38451RXS J144037.4-384658?툳÷ïy?«*gÈøB–?sràLé«?iAn™˜à÷?²ƒ?yCµ–?ª€Âòª ?î&
!LÖ?®>ȅ6á?tJ÷(Ö?ˆë1Ø5`ö?©°Ô‡F2{?¬[õ[€?ëðpNâì?£\ƒ‡9‹?'Lä˜"~?ÿß²?ÁV¡«Âß?¢{]J~¸"?æìàë_"×?©˜ÏÚÐW?AÅZ?ˆ@îþzn?ÐV<™
û?¨ër²ío4FGL J1440.9+0609?ã;‹úÓ@LJ@c^JÀ9¦K»À5À;ÿˆ}£–@ÆK‰Á4h@uv'[¸?¹XÙµé[y?®ê£§dˆ?ñnkÝËù@
'?úTz?í=b.$¿äõϏõ«é¿á̀v²å¿àùÊÇ9¿án"áÉ´¿ân@$ˆKAGNbll3FGL J1440.9+0610PMN J1440+0610?ïѺêàv?i̇Ÿ©?GeÝ_'"?<ªTéÖ²æ?t5Îãà'?h>ÝûJ?ïv»uÃû?‹õ÷q"Ön?Rë³Aé"?a£-ø?óžÆÄ+?‰ß5¦ŸÕÜ?ïFè7?'âAÁ~?l?èç"a?Y\DmyðJ?›¯%â:tÐ?3mßÈ&?íÀ›ãù·?b´ƒƒX]?ŠÏ*<§R¯?r—È	ºŠ5?­L²–æ?ŽÜþf÷à4FGL J1441.6-1522?äi.Uº@CäU•:À:M0o3"'À;ßr)Zl@&+Í@ð¶ß$¾%?ÈUÛ~ÁQ?ÁªQ¢µ?øñzç&ë&@
¾Ûc9¿ës­ÁnË?ïýž%ðT'¿èš[@BH¿åªª˜Å^D¿àCnI‰¶Î¿ïÿÿÊPËAGNfsrq1FGL J1441.7-1538PMN J1441-1523?ïÛ¿+ ?g~®¿¢§1?Qn'÷Šü?JöñIÁƒ?k‰‹Ù}:?dXÞ´ÉuT?çW¥?ˆð°uË%?PÊ}W³Ò?`F5~Ý+:?‹ø.›F€?†1qïí?ì™F¯wqû?¡WÒS?,M{`»?F?Ð»?·@ÔØXÉ?ŸŽ0>$@G?î3™À¹?âO½–DŽ?NSúzá]?nFs›E§	?«2ûä¥#?Œë¶!"î4FGL J1441.7+1836?ʹ4‡¤­'@O¢ Ç`À:€œߢ'À<}šYù@REP—@zŘûå?¿dqēm[?°:ŸŸíò?ëæ±Oí@žÍØ¯¿êéôæÇJ¿ÐõùìÀˆ¿Æ4A{†¿ä¾âÿ>9!¿àÙ O–@I¿ÛÅu€	ЎAGNbcuNVSS J144143+183706?ïl•¶#F?…`¯NÑGY?Y³ãmú¹J?MÂS"£$?Ò®«'?"ˆâ湟S?ï‹||'Ï?ˆýŽŠŽtý?Gù6±"$?Sñû"Ÿ¶T?‹ÇMpz?‡ËH¹Ö·÷?îhÅx¼z™?Ž">'øø?y¤týum8?nÆÌ]óY?¦?ԉ¨Ï?Šµñ°O?î÷§?é?W̕§µJ?tyµ|ÇÆ?bø`Jô?œìžøÐì?€¹Õ‡
üv4FGL J1442.0+4348¿±ŽÛÓåj´@O"úÖËSÀ:x˲À<¯Ä
†k¿@J,\\×?ÿzΝ‡dä?À"¡²í©?µ2»"?÷™WÚ²h@"(¶ØnÁ?î钀J¾¿Þƒº¿Ùõ)¿â!Êö2÷¤¿Ùk*ñER¿âPŠ\ô¿ïÿÂÞ6œAGNbll3FGL J1442.0+4348SDSS J144207.15+434836.6?ïÅ¿µ¾?r‡´GE"?RôálžY·?Hïrz??xc;JPŠ"?pIY=ʞ9?ï'{ò!ÝÛ?Œ$–…]?RŽ{ËÅ?`÷ðr?1µy¼?Š´Áw÷?îØNiN[§?†ä4Ãü?pZˤÅ?a}¨ezÝ? xG_ÀÐó?"IEq*…]?îõ,»c?|®µ£=tƒ?…õÖâWûÌ?k-<닃?–a.÷g¡?wI[gP¡4FGL J1442.2+0622¿‰ãoÈwf@L>@(äüÀ:_Ê?SÒæÀ;̒Ü6¯@q§£áò@"†ŸÁÑÇ?ÆXã["‹?ÔjÛöÀf@Ž†ƒ<`@vå¿â€)«|ñ¿Ð%?•í¿è˜b'+=ñ¿æô¥žµ@¿ïÿå}ó Ì?íýݱ žÜAGNbcuSDSS J144212.23+062526.1?ï?'Á%Ðy?'QA¿+ÎÃ?'Qé2_?ŽáwrBÌ?zòûÈM½š?xtæ/(Ê?íWñßØ|?´Mx¿'B?˜hÑ
&+?¨=ªˆ'ÉÞ?®Lyƒ›å/?ªŠ¿ìÖw"?粜ê>Ø?®?iP t¸?¶gf£0ˆ?žš¼6Êçã?Æ1Ø£¶_?§ƒMÆ6?êû êX?©£!t4;ð? WE=`Û?'û?ÆåÕ?¿÷\yüó0?§ÄòAo04FGL J1442.6-4623¿Â;{8…ƒ@(•¶^Ì>2À:Žö¨hiÀ<-_²@ sZwÅ´U?ÿȺiú?¸`u¡æv?"¾¬Åè¤f?܏Û_Œ­x@û-+û¿åՔ«W?ïúhai¿¼…
ìB3¿Þ<ǼAº5¿ã(qGпÜk:¡±SAGNbllSUMSS J144236-462302?ïzàdwÏC?‹7d=²?YmÄç=´Ó?U,®°½f?Ž.E$xw?Š¤aTo:?÷¦ky?äòâ€çà?GA9³Ø?[ۀ(ÌÇ?Š¡ŽÔ&h?PŒ=_1?î<ÃJ+?"*ºRó,±?u'‹ÎŸ?eC
x6ÑQ?©ƒyå&?'ê¡0¨õæ?îÂV1<(E?" ""*ç?}á0ö]?hã¡&4? vÍ{¸_?'.‰˜Ó³4FGL J1442.7+1200¿Ý>dÈ4?U@MëöÂiœ|À9èóɐØ*À<1<°Švç@ €&˜ðý?úÏÀÒÆÓ?¸Äßîg§.?¼'‰¡m½7@?¹£ûk@ÜíUÔ¿ï¶PÕÛi?ìyK!K¿Û±EC_¿ÁwkFud¿âï6ÀÁ&¿Ù¤4'NùbAGNbll3FGL J1442.8+12001ES 1440+122?ïÊ]Ttß?p©bQÏË?QFèY"2C?LqY~j?vÄ¿d""?m—?›Së?ïM¼~Ñ®?"n,&ÝÁñ?d6*.Nw?v¢¿Ì$" ?"Á¸*[øk?'7Ӎµ¾?îhÊ7lk?ŽœŽL"+?vy–7?eè‹L"Óâ?¦±zíeæ‡?Œû©zd?í6
º(¾†?'G*•ÓZå?–àâÃ"Y?€Q'BüÝ?°—Y}ùCA?ywÞ±1•4FGL J1443.1+5201¿ê¡QFÍ!@L¾Ç¸Õ¦À;X"%"À<ä@¨f»÷@È,å'?ÿ,^YQ«?Çw*Cuu£?ÀåOe´?øÄÉþ¼3"@*0aFÁÛ¿ÆǪ5¿à\¶úS¿á䠓ˆÞ`¿ß"ãÍy¿ß™Ì$0`ñ¿ç/Ç~fAGNrdg3FGL J1442.6+51563C 303?îª2ë•ì?™6«åzj?qpö±¥g?gÇäyÈH?£.ÀkôD?˜$í#.Ú?â0vk? É/'ÉÈ?o)@[k¯?w(KÊ1*?¥tÝ×Aé)? &ÒªÔQ?î	Fç¡Ó?€…:¹‡ƒ?vÀýÕ½þ?cíçèæËÛ?¬"qåÈI?e
vˆÚ´?í>wêÍáÓ?"ÉÇô¸ÚØ?'¯X¥Ïß?}É
ðÞ|¢?± j€K½p?"PÙõ–·Û4FGL J1443.1+4728¿Ãä8èî…H@N&ԀuÀ:k"Úí÷ÀÀ<¡´¯Ÿ•\@r*£Í@^ïCðÙ?¾a¥'°?ÈõæA½å@37º@Ó´Ï*8¿º^-ݳÏÑ¿å¦Ï!»¼"¿ç-O>+´º¿é©ŒUä8#¿ð?ïæþ!¯AGNnlsy1B3 1441+476?ï
툥t?™×Ú=»?›Ò!/5u?"I±FìØ?¨ËµsÄ9?†rg¦¶¦?ë¿UЋÜã?ºËE]µù?¥ãÈAÈÌ¿?®_,¹ùàï?·mZ¼²"?°v™¿£€?ì"5®aÎ?žžÿ™Åú{?žÑÝ׃iE?Ž©+BÝi?´)ߌ¬??–æÑU=ÐÂ?î/ÉÂBTq?"è^Øò5?¡…†˜k?¶.öäyR?—J…fæ?ƒÔ÷ÄÙ(4FGL J1443.6+2515¿ëæK-GXQ@P4t>–=ÅÀ;-ZyɺÀ<4šöå¥@#

éw¨X?û½{Uá³å?Òð'ÿ¤:‡?­•9•T?ð'ß»¼Ú@­pՀ$©¿îÖëÔÏЍ¿ïþ(ßó>?ïû»'w"?Újµ ¶Cs¿Ö£D\¿àŽ¿`}™3AGNbllNVSS J144334+251559?î÷øáÝF?¡§˜H*¡7?B;Æ×L"-?E‰Y™éè)? 7'Ì"ùb?¡{¢B£åô?ï¯û.!ü?«·ƒ¡"·3?ZúÙi'©?sâb
!L?œºSª¸=?«ªD¶YO?ì FÍ`ª?¥bjۚS?lŽb'j?dµ|®?¾YŒ×›?¥b¶lô?ëú5td'?¬Õ©^UÝ?Z›¯cùµƒ?^åʯ²kì?¿Ãå¢ôž?¬Ê?á}4FGL J1443.7-0954¿év¢žŽ@FlvJßøÀ:ÜdöúÀÀ<hô'
´@™Úk›…@\}ÿà?ÉzúÁ»!?p:ÙâãN>?¦¹ÉdãY?þÚÛô#`?¦É{ßto>¿éžÒ¾~Up¿â\~¸+¿àw@Ý?â¿Ö6h½ÕG¿ïúua«ì'AGNbcuPMN J1443-0953?îD¢‹Üä¤?¤°èz·ï(?cK©e'£P?ZLãxOx?ª«Ø›'?¤5ê÷Ò·?îç"ÚÕi0?šô¬ü·×?[dì+ƒ%ú?e(«L	æ? ¬ŠñMS½?™ä°Ä†?íW~!žUH?—Òo‡¿S?€T*<`ó?lF"ó°9
?³9‰«E€?–M]†ò ?íœø'¤T?'ˆtCä€?sGÌÀ"×<?dV tÕº?¶N›oaí?'c1;h<‹4FGL J1443.9-3908?Ýé30à@2µ÷øʁ™À7ë府mÀ;8˜Ä@\a¾¶ß?ûÃ/zA¾?œ¼åN"ø¨?¬ÇïBmÍ@ˆ®`Ðû0@ í6ϟæ?ïýÖ.u^¿¸ù§÷*ni¿Ûà«;'¿Õ'€áü}¿á8 m]Ñl¿ÓÜ.ÿò¾úAGNbll3FGL J1444.0-3907PKS 1440-389?ï½0ª~'?vý'¸|C?Q.³òc']?P†âõ0?}E.'Û?u-)%LF?îOˆÿf;c?ªb`n™€´?‰¥"i:À?–D®ìû?¤žïMÈ2?¤$16l¨?ížÆº"ÐÑ?¡~•Ó>©?Š,\Že^?…º0J¯éa?¯ˆ}3@Ù®?Ÿ†›–3†Ä?ê@çðEùl?©?Trü'*?¡Áª›ú?ŒÜd,õ
ß?»/÷ýsQ?¨v'õ¬X4FGL J1443.9+2501¿ïÿ¸~ÙqB@P,†hÍÀ7Ðe…•Ö–À;]ˆ{¯¤@ûV$#öª?ÿwÃ Ô ~?—	"ŸG¿˜?¹®œ`w	@!ìæŠ
5@ù$ƒmj¿½¼O?òøõ¿Øó¤·Yô¿ál¹–m•¿á¢9ìN¿æµ6]ŠÒ¿ç_û¹IbAGNfsrq3FGL J1443.9+2502PKS 1441+25?ï·<m
|*?‡}¾w4šg?Oˆ³gͨ?WØ®ö,f?€?Ü1jx²?†°»fªÊ?ïW«@Où?–‹m¯€ì?c{,×!þÌ?xÃî͌û?'›2[:Àó?"'{Hît
?î˜g¥t•?—ÑŽV$""?Üâ
o?Y9..s?œ)GhGý?'‰aë²-n?ïÙÑýö!ã?g)\êÒ¡ü?8±1ÙØ?3«-ôL
È?q•ÐIÛðü?fdQ0O'á4FGL J1445.0-0326¿ëßҋR®ù@Hw @|ÇÒÀ9‡9+
ËÀ;î¬yp@ å"aÎüþ?ù¶ï¶àë?·sJ$'YÚ?»¼LÞRD@Ôƾ•Òe@"N÷3þŠ?ÐÉ@üžý¿æÛ§r$¿ÐúAd¤Dm¿Ðí»Ú·5¿ÒK1­>½¿äv‡EÙþäAGNbll3FGL J1445.0-0328RBS 1424?í·Ó£­5,?£Ñ,"s:@?†EízG)Ô?y¦mÿPŒ?®ñJfšâ¹?¢ÖhiR8?î)ö=?¨³í¿|?ƒ–×@†P?#®N´4?¨‰Ï9½?£Õ7Ù¥¦?ëg[†0Àè?¢¸J²a?–‰³SÛ¿x?‡_•ȥ?¿"¶ùƒâ? ;üŸ×‹_?åW¹}îÉÌ?¨…'"ùôƒ?z—^žè?ˆ[±­'ïz?ÓxãŽ8}æ?©ò…Ÿó4FGL J1445.2-1954¿ïž½ÜU<.@A¾ýq?À;yåŸ+ªÀ<r`±¿Ÿ@öé·>E5@AƎÅ*A?Á&Ž_(Új¿¶û`‰ÆÕ?öRXâð$Á@Û³'ÎÒ?Ú'Ý¿ŽJÜ¿æCx$Õ¿µ7ýu×s¿ë)xŸN¿é*ƒ–øÕi?ÁóTöÒYÕAGNbcuNVSS J144511-195853?íÙ¤¤ð¤¬?­f8íEŒ?'!æFh?¡¿…§è2?­ÝrwdI?§7Y(6Ï?î½áɝYX?¡1X$?k–EÞÎÄ?ziFàuÚ?¢h=Š?žw´ù›½/?íºz¼¥É÷?—§½îB¢?ƒæ'¡¨#?GíÉ6¸?¯^¯Í9WØ?"òR®­8­?ìíåêâ??œéH˜ÒN¹?xìrözŸ~?r5EV߸?·	€yD?œq×$(jQ4FGL J1445.9-1626?ì#ÎÚKÄ@C(˜ëÀ9ìã.qÀ<õHG@°jœ€ÿš@•öâJ"?·`oA{P¿¡$`©ÛS?äg]Ж@Õ@–ÉÁ¿»ƒk.ø¿é–ãô5ǿ䟗_'œ}¿ä dŽõÑ©¿ì¨þoH?½¤òé.–AGNbll3FGL J1446.1-1628PKS B1443-162?ïªÕ8¦®º?€¬©Ê
¿?g›â×ñ?bYkª?~ÇÛ;Ÿ·M?|Ëz	hw?ïž|«È?ˆ#:ÿ(Žö?D¢îœûmì?WoHÊ Ú?‡Ïëk×%?‡7³p×)"?îðãFk@?‡§8o‡ù—?u8š'|i?g†às¾E?œ£	Íøé?"ÿâUv"?慎ßÏs¶?l΀-™?_[ïg‰?M¥óŒ_¼?rŠ1ò?i˜È¸·9ó4FGL J1446.0-3039¿íjå6َ…@:
§;BÌ-À:ó"PXÞÀ<nsGyB@õq´ùŠ@趽–Îä?ЯûIaô?Òcˆ»zêØ?ü|MÃØ1…@"Ì€KÀ¿ï‡Š¾4ƒ•?ï¼ë
)´.¿Ù©`J{¿èÕ@8Õ3¤¿ì%ƺd¿Ó/K²…ùªAGNbcuPMN J1445-3036?îӔ–ÌN?§‹AŸO‰?{õïÀî??v÷껉¼·?ªÔÖX?¦ˆs92ßí?ïw/©wÔ?"'œšÅ~x?ZÆÅÝ»¾?u~-K©7?ŽÛ=óx?ŽÙl=HÍë?륩°d‹? –FAֆ³?§" È©!å?"ÀØG¡·?·¢ŠŠ·?™‡ùæàMP?ï=›>|¯?}É_M–ûo?hÄ"+?Wê=—)›?•4Þ¨õ?|ŒºË+4FGL J1446.3+3111?×5Ç~"@P)ú—á2µÀ:¨ñ-Õ%aÀ<©Êbh@rÝ4y@Sw[0?À&ágc'?'ùXyœVÁ?ÑÞ¸ù6@û0ÍÓ2¿Ö¾ÔãÄ¿ßâ¼Bô/¿æ"º!N"G¿ì¦á€¸ø¿»ãÆÃö¡¿ïô½±¦×AGNbcuMG2 J144640+3110?ï´!·'½?˜/ÍhK?V£åÆ&?s·¾¢ö®¯?€7}ž—×£?•ž-_›s¶?ïÂ&¢Î?€‡ýë€ø?4lš~Ib?HÎÆDrë›?}¥÷uM´Ë?€7ÞyâÓ?ï#V"Í×?…–9À\Ö³?lÝhÐ|̳?bQ;IH/?›ŸèV«›?"1ÈmD ?ïùõï<ãù?9ƘœÄå#?#Mq¿»?ñ	…
I?F6;èýe?9ÐÁfn4FGL J1446.7+1719?ïÖ'žs-@NÓ³áC|WÀ:²ìzçý«À<s›x¦@Lȯ0ړ@äÖä}Ãz?Ä#-¡?¹zþuÍs?ðítw¡!M@–më?ïá\Üyèú¿àH8³¥´Z¿ì4á=òÿ¼¿×—ÿ»Œ‰¿ë{Háa«¿ðAGNfsrqS3 1444+17?ïë!M‰$Ÿ?m.#ØÝy?He
´ɐ?j 8^Iދ?]ŠßŒ\\?Xfÿï3
¸?ï¥Þ'ŒC»?…÷B`8©?E׸ԙŠ?e⁀°Kþ?…*ु?"G+B^T?îÊr´u?ŠZI‹¼VÌ?u˜Å!Àœ;?ož<H­? ¥ÅÚ|¥-?‡¤â~þã?裏†"ê6?mñ'ìðÝ?m(ùÆl?\ÏÛ4":?}˜.8§¯J?g#y²¤ƒ4FGL J1446.8-1830¿¸"™Oäµ@B;½‹ç)À;·ª%ÙÀ<†šÜ¸o@ N'?ØÞ?þsŠ ÒH?Óû–
óފ?°-ÜP§?Üٗ ¢‰@—ñ¥]¿è=.ߑu‰¿å©ÊiE=ø¿é¨@[9âz¿¹B	岿ҤvÂT"í¿ïú Ë®AGNbcu3FGL J1446.8-1831NVSS J144644-182922?ïf) Pï?‹a½ùàƒ?D˜ÐÒ»'å?:Ùééë`?'–oiåF?‹2"áÌÄÊ?ï›X
F?ƒ–ã¥D‡?:¦€Ãö/N?FÒß­[ù?ˆTÉZÍc?ƒdßV¬ÿ?íü–¿šu?'d±	ÉóG?soÚ'bd?aŽA´Þʪ?­Ûø˜Álm?oþOÇJ?îÄ욟ö?‡¤JÅãün?L˜ðQöçU?Fwë9±%ì?£>Û%?‡ç"	ý4FGL J1447.0-2657?ëûÉýQ@=09-Œ*À;‹;26À<—)2ÿ0Í@ °›yB·
?þ³&Ó©_à?Ç£ue‡Ä/?ªugáÏ×?âNæíàBË?þ³a'È?è%¼£n/¿ïÿÿ)@k*?ïÿøsCÄ{¿è©ý·{W¿Ù,ëñUB¿±Ó	&ð.ÒAGNbcuNVSS J144657-265713?îÿZd•c?¢X&JÍá?KTìÌ9'?F£ábRÿr?Ÿ:+Šû?¢>²­÷ê?îÓ8ìôþ‹?Ÿ|}qtÔ?g?=Cæ¥?tˆ5Tô˜?¡X}_ûØæ?'ßWïï?ìà"Ò£óŠ? ÁíYA‰?xnö"—Dß?gǧOíæ?·tj–ï`? »\4<j?í5ûÊE?¡<Ðp:ú?xƒðn}ƒ?y'ÇK5N?´Ï·¦ì+? Ø­'þ}4FGL J1448.0+3608¿ë5,`õÒï@OÛKƧïžÀ8é™ÛøóÀ;¸˜SH|q@g.†?ù˜Â¤TÞ?ªF-ƒ=Y?¼üë"£C@¸á]}Š@	¸¯&Ëî¿ïb²|¿n??ïþk«IÅF¿Ñ)õœÏ®ÿ¿ÚGž¿Üí:*ž9<¿à®!`¢ØAGNbll3FGL J1448.0+3608RBS 1432?ïڕОՙ?p͂cxý?W$uê'^?_ÍÃFÇ~5?iØ.&5Ð?hb‰Uó2?î‰pþò§ñ?¥ìÏuW7?'jr€ʯ?ŒÅ	îŽw©?¢ÎSpЎ4?¢T|û@_?í:2D ,?¤¿ÃÍޒ?¤,=çyù?š+©zæ¥?«°ÇփL?›¿ŠNÞ]?êÓËV–6\?ª\.c?ŸOy?ŽjvUª¸™?À¾ï…]7j?ª7×,ã1s4FGL J1449.5+2746¿íŸTª.ð·@OìÏÃøÀ;ÐÄv¼õ¿À<øV6mzW@"ox.åƙ?ô•|3WEa?Ø\Kz§»ñ?Ù]لÁg@¶ÄŸä@µréµ?¾¤çÀîó¿ÝI¼ÈÊ?ïýÐÈÚп¥´£5NÁY¿ÒT9]nÆ¿ÛîH}GS|AGNrdgB2 1447+27?î/²F¿8U?¨Ø´–û
?ŠquxZ"?'
dZÅ?¨¢?6®d?¦z£6L3þ?î`#€"ÎÛ?¬n/"Nè?vZÉ|ºUv?†~Rwr?§2nÎ;DŽ?ªç€ô[¼?ì¨ŒGß ?£ê³½|n?µà–
_?˜МÙ?»mCv[«?¢zÃļ;?ë‡ø~J3?ªx;!Í]Î?ræ^à²oè?qkyt¾Ùk?ÁHëÑ U?©ó¹ÜmK–4FGL J1449.6-2137¿ï²H#±@@¼Èÿ¸²dÀ:»I»4ôÔÀ<Kžã…uö@çk´"@eäEVJ?Â-`‹[¿«9s'óS¹?ê†nCªz@Òùæ‹dο×ÈçDÈ1¿âìÊ-¶°¿ìÉv7]d?±å/D;CM¿çRw@Ý@¿ïÿ‰XAGNfsrqPKS B1446-214?ïéMµZÐN?h¸\?ø×?Aœ(|€bª?@ߣ\€Á?bK@†™?f‹èƒ«?ï»0@`?€@z¶êÄ?8ôÔ]ìû?J¦ìh¡P?€shz?W£!†ö?îãï%dK?ŒG«™È?hYœð âr?b£›äïÚ? ;sÚ½½)?‹´›ÄU¡?凉ÉùöS?rü疴%?Nfˆî•&æ?GlÙâq?"«$ò™ª?r"xšßú4FGL J1449.7-0910?ï+RßJþ¬@EÞB||RaÀ;)!°:À<‡àmòL@ >1´Øå4?þ‡S–€	¦?֝ţ7Ó?»Ž-TÌàï?êð äÑü?ìæ¹ÏçV¿ì§'Z¸³:?ïþ¡€Ã´Ë¿êéˆÅ5ÿ–?³=ïϱ-µ¿ÝÐ$p!Ñ¿ïÿÏ=ÀTïAGNagn1RXS J144942.2-091018?ïÜ@eû'?Œ¡%!r…Ø?.úV‹#Çi?3WPÖ:?pçúN#Σ?ŒœØ†¶ð±?îä–9ˆû?Ÿó>"Æ}?sx­§Uµ¡?'(YR¨†?žùsD?™±ãJÿ×?íì4:žU?"ny/…?'ÊW2Äw}?}â|ãk£c?¬Š!?¤üË?'4`νüE?ì…›að?¦Šo7ì?—âÙç"?"_»M;é¸?¹"Q.v–Ô?£j?¹Ñ4FGL J1450.4+0910?îçÚºv3
@LT°ò{²ÿÀ:7s	â×ÑÀ<e …F%~@´—Â;ú@æ3
9?Ã
'åÍúŸ?ÅëX¦4]@&¤û¨'@SF¶È©}?ì!åbÅÇö¿Ù8¸ãá¼H¿åÍà¿åq•n'¿é{NP¿ïìŽ:AGNfsrq3FGL J1450.4+0911TXS 1448+093?ï‹>"ýîÌ?Ž«ÖȺìL?e‰;»?b¢2p©í˜?‡î8{?~?‹ëè@»Ï¦?ï™iØ]Ï?…cºþÖ ?HßTo‹…?Z.«Î­´Å?ˆ1°H¡"?"8·MXö?îx³ïMÍ?'Q¢Î—¥?ƒ'¤QŽ†œ?x¤Íå»y?£"%<§–?‹ÄWžT1?ï±®rí"v?iý^ùŒ0?eǕ¸ƒ?R0s`Á>5?|Dû­7a³?eŒ¡kè$x4FGL J1450.8+5201?Öùd•<#@LEåóöÀ9¯UªLoÀ<P)µ/ë@7Ž`U€:@ ÷üü??¶2¬`×ÂZ?¼ŒÛ›Ï¿@5 üÏÊ@£þ·Öp?í/B]r¡Þ?ÖؽÜD"¿ã&??#€¿á*™Á²'d¿áÚŸ‹Ëü¿ïÿú÷''ýAGNbll3FGL J1450.9+5200SDSS J145059.99+520111.7?ïip¢¾ÏŸ?'h`*¼id?y«ÊAwۛ?p½z!R®?ˆÍò/*5?{~Á7\l¹?í±Í™6>n?°FlkwZ?"áZpÁÉ? 3@Aö?ªòy4;Q:?¥0òbq?ìϳvª—? Uý€Çq?•z¦ÏÕÀ?‰9°@0¶%?´#º–¶>Û?™ºÓǑa+?é
ÌCøÔ?©öÎ2´A?ÃNÿ­Ó<?¨Õ`ëh³8?±'ÿàÞ<ç?'Qƒœu4FGL J1451.4+6355¿ïÚÄ'.:@H:A€ÓÏöÀ:ƒŠc›±À<¦p‰Õ×8@ "6}•'?ýNQÒÓw?µxõµ#bÜ¿€ÂZï
®?Ì©3€
&u@à±F?ækҁA³ÿ¿áŒ&ÿÉ#u¿ß S<h5¿âˆéH-–;¿Å€¢è!çܿʹÁáAGNbll3FGL J1451.2+6355RX J1451.4+6354?ïÝÀ¢Ò(?mQ0"Y$·?@6;ð®]?8¦9ø[?n?Pd1¬m?k}ë4›}Õ?ï®b
Im?ƒ³j$†xö?6™<Ü}ø?Gí":<ÿ?ƒ³®†À©?ƒ=ÕPû?îÉ÷fâR?‡{;j?eÿ²B¦Á?_žÉ$õµñ?¢M–¶´¬?†ËÚˆGÇ?ïƒcþ¦P
?uf©Ès?MÍ×°¯ê?A7õ£Ø?J"ÛaŽ?uQ>åvðy4FGL J1451.5+1415¿ÆÄÀ†9âÇ@M›ÑþdõMÀ:ˆÒÿì´ÊÀ<wí4Ka'@'{yž@ݖÁxô?Å{>û…i?Ò¾ä!'B@²• Ž@ë¾(DAοî‰þñã?·Ð³Œ4c¿åGªfpw¿èOø ºÎ¿àLèyÑ¿ïÿçvœ>AGNbcuNVSS J145126+141626?î~.y¾?¥Î­Ùf?ˆauä)Â?Š­¹ ®;©?©Pĺö©·?¢ˆÎ¬¥Èá?ï
<\Hl?–+˜JðÌ?hù>ž‰?ṕQ¢Òï?›™Tï¦?"ýUg
ò'?ì†Ø"šÃÄ?¢QUKý?¡î–Zيi?'өܯv??²Ñ󽽬?™"èË7?îI¶‡dj?Œ}gWÿ¾—?"ú"67%…?]AéûRÁ?¡gMn¢Ö±?ƒyQl¯êQ4FGL J1451.8-3851?ì;—±É!ƒ@2FìÔªÀ;qߐô¯jÀ<‡ªhô¶ @ þGG<Tš@gã'ñ·?Ì+ýß¿BÌ?{E"ï¥1?³\&á/?@Ùt·b}¿¦<!•.®?ï[›fù3]¿éÌewS¿Êz:ßO¿ïÿüÚ±'Þ?ïÿíÁ9ÔAGNbcuPKS 1448-386?ïÄÍÃV,5?wjT`5¹¶?TÊóétç?[—ÿfä¸(?xf×ï‡Ô?tt1d;ݼ?îáuCa©?¢°±"HNQ?e…a›Áf?rúüK½ð5? —W%°)V?¡Ûð'Â¥g?ìäËÙö¼?S¶-ºYÂ?
ìÖ/ߒ?'*à¥+>Ò?´÷énjN+?™ª°Œ®=?írU~h.ä?œKgI=yx?ŒÛSGôÑ?ƒûjGð|Ð?°Ñ飿î¿?›YP
ðz4FGL J1453.0-1318¿ì¨¾ôƒ0]@CøŽ£œQÛÀ:Ó Z8[À<Zê'-@Ô®¯Um›@^pc?jy?Ä:šE;¿ŠðÉZ7À?ÅçúîHH@ñp;Ò>&¿îPáϓPª?ڂRÀ—4e¿ìJ[¾l·¹¿Î0CÐí¿å/5B,P¿ÌT—œiW²AGNbcuTXS 1450-131?íöðölzœ?¨¡v¾nö8?oˆFÿz¢V?n´Ã£"?®˜l)@¬4?§º5QÕWg?ï5Æ,H?†Æ7IH?AT'Ué?RÁ._ÆïG?‡Lè­"?…ï'Z³?í†ëÇmìÆ?•àÑá­?'O‡k"A?q;´÷öÍx?±~À³£5œ?",C>ó?ï'"5?€¼ºýÒµ?kaG­K?Z@"6ˆµk?˜ºn.惩? KÊdbX4FGL J1453.5+3505?âÓ£ç·@Oeì,äd™À:¸ŽS™ÛÀ<µ™ÙZyÉ@#>Wÿpc@X*™0¾?ÄeqH턨?²´rˆ2¿?꿹SsD›@Z(*¨3?ã¥L?ə'¿æ]4Ä,ë¿ä½Ø"kdÓ¿á»2Ál"¿ïæõ½†Þ¬?ëñø¶Ô"AGNfsrqMG2 J145315+3506?ïoR$M°è? Õ
äDB?^ß>%æ®?dÖNp³Þ?'Ǖ‡""?Ÿ¢Íaf™s?ïž. á
A?Š+lUêF~?BÝè[c?UKƒ•«‰I?‡F™B??ˆíú®ÞQ?•
;?'­5[X?wz¶b±º?jûü\%yÃ?¢x'ð3(?Š¨!÷{ý?ïß6l+J"?YßM²6®R?NâÄÑöI?@A˦ItÍ?iâ 7ì
?V¬Es¼ÂE4FGL J1454.0+4927¿ïãݘ›Ê@LÉÛ"Ðå`À;Lë8ȞjÀ<ª"Y–tK@"…|V'@¶LãÞa?Ó­Cðo¿?Ñ#l`üD4?ùìúÕÔ&@GÍ`Æi?ïõðaýK¿æÒ¬X4õ¿êÕï ·E&¿ÜjÃQ#¿ïñ'L ¿ãÈÏFúTAGNbcu87GB 145232.0+493854?ïÊ=–Jó?t¿¹Ã+)Ð?eÎg³õI?f+f‡\Ç?oô¦YZ?l "!ŒYf?î2 û¥Í^?©·ç0?ƒ²?'#Î¥Ã|1?'67|°à¨?¨Tüœ2K?¥´ô`lï?íÈ"€Wæ?–¯ˆÈmE?ú £&?ƒy^S‹`,?«>©‡*0?…Ôæ«?íúÓñ?'"(RFC
?'\RIš¡?~$v-{­î?§¤¤ù³Ÿb?Ófµ_–4FGL J1454.1+1622?îÊb		"ý@MÒ*¡"9ÞÀ9ÞúŒ"¹À<Zjۖ"@OÞÉ# @T[òoÅ?»Ð 쉬?Å`€Þ·°Ü@žÒ¾~Up@©§°Å?í>aå£2¿â¶œLÒA¿ål(—9¿æ:m"gÙ-¿ëæíª'æ!¿ïýÝÑ×ÏAGNfsrq3FGL J1454.0+1622CLASS J1454+1623?ïO
ŠL?'L÷ûFbÀ?{¦L›é?uTÜk¶?'Ym«·?xwá
úL–?îþV"Ìá?¢ÿKdšŽ?wîÝShéÝ?•·­aËKâ?š9x¢é4?•ìQ>å«?î"6u]©t?'JÝ^H?‡O±ðí=p?}2"L¼îW? è¬-êj?‰þ–O,ö?îQ#ª:F<?‹&SþsB ?Ÿ*ÈO(¸G?"ÌÌH™Y?–°ÂiŽ€%?|—_‹ö5W4FGL J1454.1+2647¿¬4à³8Åý@O[2ßP]À;,7–oCÀ<°ÛE5"7@ØâÇàÔÂ@çÔÅ¿'R?ÆÛ Ña?¤Æa½y?Ù.$Àÿ?óT³.@?ïÉ,.\4¿º–ØÊü¿ãp,¸Å¯¿ãd¤úö«Ã¿ã îA灿Ö÷u'c/AGNbcuB2 1451+26?íئƒ®{_?©}¢2|™S?o'¸²`¬>?ejÚæŸ7ÿ?°>¶ùž?©
ɓüýo?íEÝÀ¾Ìü?°,á?N@j?W8…Fn?–Ëp€I"?±»C؆ˆ?«Týu#Q?퉦â"ÐŒ?•ìJG½?ˆ!âEª§Y?{"¬É=«Í?°®Œ¢¬&³?'óyYA?é'SS_do?¡í©båº?°ûñæl{?˜Ö#ƒ–?Áxº$8?Ÿ¬µ>aÀ4FGL J1454.4-3744?§—Eb|û=@3ÄüóÀ9µm¿öûuÀ;Üz¤áÌ8@ Ç†>@Ñ÷" ³Õ?ÀVË~C&ñ?É«ÿbKN³@ؖdZól@cô?ïê<´¼4Ï¿år†?tµ	¿æƒþý¡€ï¿çñLÝÙ¿ï÷Œ^G³ô?ïeÞ×sAGNfsrq3FGL J1454.2-3751PKS 1451-375?ï¨oâÞÓu?€_VÐ<?z$˜dhn?x»*ã+Öf?q£v,ÝR?o垍^ä?îÆ-—î[Ä?£¯ÒÉ^å?|#=ÿ%?‹oؙ§? "vƒä?œÒni7™È?ìïµËüuu?¡Xf˙Ó?£ïÕ;g?–ú%³nœ8?­è‹PcmH?"8q!òʑ?íޖà¡?"dÔñ†a?ŒÔÖt?yäLÐʹ´?«ù\u¯?'Úª~|¦4FGL J1454.4+5124?îš1i•¬@L9Âã>ÿÀ8«]|OÀ;pêWøš@"3¬?ÿ~"Ô]ºÆ?—Ù~¥¼+"?¬f¸#{ï@¹¢ž%•@ô½:ˆ'
¿Î4
H®D¡¿Úp.›ô½­¿áßÀà/€ ¿ÝâÉc`Íu¿â‹ÑŸÅW¸¿ãë[-M@AGNbll3FGL J1454.5+5124TXS 1452+516?ïîVp‰Õ?W"é:Ø?6pñÂ\È?10Ìǃ´?]¶ãZU&&?UÁI"Ãå?ïZßaԉ?—
‡ç¨Û?]›[ÊÒC'?lꨌYÿ?'ÖNWJ¸?–#Ój?ï1}Táõ?‹†Û4$Y¿?wlˆâ̵?u]F˜(­?"õ3DД&?‡:Þ)+lá?ïÇDı¾¦?hrQûÈZ×?O˜ÝF]Ìå?@œôjØF…?xjþTóg?gJŠ}æ'4FGL J1454.7+5237?ÀqÚ¡)c"@KÜýŸÓo~À;=*³1ñÀ<Ö»ÉoJ;@
—Éà´5?üË;¸<òÐ?Ô¤Kc֔!?ÝuX<8@•0¸/@9Æ7‡UÊ?ïÚ6ýÃÞ¿ín_E°¿ÈÒ<ã¶^¿äÍ _Š¿æó|†¿ïÿû˜'2AGNbll87GB 145311.3+524904?îqM@_Ü?¢Èï+¹Œ?ƒrbÞí?€zpIÎÔÕ?¤"t
¶?¡)o'>?ë¬ÙQ`?¼HY0'?§å×ë{y?±vAÔN?»7­A‡¸v?²ôc»¥xà?êÚø$JšÊ?¥¿ÐÐÒ8á?¤ÃøìÃô}?'¹kèËc?¾ÆBgI/t?¡‡ãÊtN?çB"z,à?«Æá>@–?²	³¿a"?ž p#¾í?ÉðÓÞf‹¾?©ÙrIçÜo4FGL J1455.0+0247?èÊôŠMm¾@IÜ¡ô±îÀ;¢oþDÀ<ϓ¤£@ ïþ¾âSr?óDƒ½B(?äF
<ã?ïýfÞ"N@dä]ã
&?ô†²+‹Éø¿ïÿ¾ýq??ïÿò~#¿?9Ár%·I®?ÖúÿšÕXâ¿á*Ä>³Äé¿ïþÔãÄAGNbll87GB 145233.9+030210?îûF¶E]?¡Ç"¾Eܽ?…7r°üî?"õn
‰+Ç?•ûoçyGx?Ÿñ$€$Ô?çïr{Ôå?ˀ&ÔÄÈ'?Áéۄëæw?ÇÖæ«*"?¼°µ
ô?¶/a'ˆ{J?ë‰)F&E?¥I#1ýA?ºaý%'?ŽÅ¯ÂÛ(\?¼HL½i•?£/̨™¼r?æƒ74:?»6ÐΨ×C?´â۞^'a?¶»éܝ?ˁµ`pFh?·†Çv1èŽ4FGL J1455.4-3654¿àúA-á~y@3£åÙä"À:K°¡šÀ<Ž`€s@±®MÛ«@ç]<9A?ÁPrß­?™Ôco. ?ÙG…5@èe{.õa¿ê6Ù{0øÆ¿ã'^aŠ3 ¿é©?^º z¿àþ壞U¿ÝhÚÆ_ ¿ëš	`ÑÑïAGNbcuPKS 1452-367?íÚ@ôO‹?§e¶D±WR?€Ä
jT?w³Â1iv?®*íd¦À?¦Sl"ž ä?ïJ‡o9«ù?'*Z~ç'?U¯"?—?d/Fó¬Ê?•T"¦‡—?æf×­8?ì)ueä'!?¤GZ҉¾I?'˜7Ðv?ƒ{ŒI\s?ºPM*ÐÒÙ?¡¶6ôóâˆ?íyэjôµ?'…þ¯˜žù?uKvï%˜?bàp{¸å?²Ü¼3Yh?'‰ë™4FGL J1455.8-7601¿é5îñ(»zÀ-ñk¹Œ~(À:ÞUNæíàÀ<ß®PàÃ@ ¤£e BÖ?ýóžÈ­ƒ[?ÆÛC]!ï?¿–ºÂM¬?óËg†ø­?ýÞU·¿ãLÀmBùz¿èYõ_45¿ÍáS¨c¿á¤Ó‰p#¿Óz­%²Z¿ê>¨çë6DAGNbcuSUMSS J145543-760054?î2͹Ârb?¤nú˜âÚ?["Q·æ?QÁ!´á'È?«ö‹qK!N?¤C\`"÷?îS|¸'5?°°1¯Üµ²?fæ»5Atú?t‹<­®µ¦?©a"Åj?°Åú U?íÊ÷ÚlX?'6%ϗpê?s'E¸ S?d@ÿµÒ¥b?°uÑñ.?''5‹?D?êy4XŸ¢Ò?£yŠ É ?ÂaqIð?rIÇꭑÜ?Å"°Šuêl?£"QÅí֘4FGL J1456.0+5051?ÇnPtÓx@LG¾ýqÀ;n=þhPÀ<œVœÄÇE@ ÿ‰ þ@Â%ĵ§?Ç;«&ß½À¿§°ÉáàÛ"?ä¾4^'J@JT·è9¿ïý»íx;?ïþ
A¢a¿¿ãARz÷#¿ä81¿ë'á¿ã¦">eìC¿¸,+×õAGNbllRGB J1456+508?ïKîX{?"ÓGìÞÐ3?Wm
ÍyÛ÷?PJ`,‡m?•l8(2ã?"HòÂÂ\?îî™ÙՖ?šû5‡\Å?eZNhܱ£?lj¬d4‰›?Ÿ{i·!?™Šâüû 3?íÕß«Z´?'N_£Xë?Šø®×î?n¯‹êL'½?®°¦8–yÊ?ù¡<Â?ìsœÑ¾ò?¤]˜Tf%?",3t%Ö¾?‹+#LÏÇ?ºIV<h'Á?¥Ó/sä–4FGL J1457.3-4246?ìGً!0Ò@,¦‹¤ôÀ9'Pi¤ßHÀ;ú²÷8±!@4&Œ[Ãu@A¸œ"Ý?³ïîÿ–gz?¤®
aOG³?ì½7Σf¢@N%zãËí?é-¹a5$$¿ã]Ûèɂ•¿è¡ð€0<¿ä±¾>¶ì¿êhhŸ%Ë?Ëgbû!ôÇAGNbcuPKS J1453-426?ïÁè—Lɨ?y
`Œ·°â?L]hõWŽQ?E$%ȓ?{€:ð:?wÍ>¹üS?ïÌÉfœ¶h?}¿^5H5?5T4)Ñ?QJԂÙ~?xF	ož<?|=(îÍnJ?îtØ阑™?6: z?'—pÈn·>?{ì{Djq?¤•4[8?‰ýÿHŠ½?ïëéUè%›?P;r??0bˆ	Xî?!E[?9H?b
Y¯GÉ?N݄KréL4FGL J1457.4-3539¿ïüEŠÆ@4‰"àÀ8(¨(÷À;œÏ¥©r@f'ÿ"Û@fö^–ŽL? )¢].ü?ÅË3²Ù‡@$·ëО¥@ÓH{ÄÇp?Õ/F߸aÜ¿Ýå"ä±oú¿ä•ï ·E&¿åȖÝ&·¿ëwöaÍ¿êO'‰²›ÉAGNFSRQ3FGL J1457.4-3539PKS 1454-354?í…-–ÞT?¶w"·Ô@-?¢é'='oü?¤©õx³çÐ?¬^éªÙ?±›GýEu¬?îøñüʟ?©M"®B–?v³ãïÞ?˜ë̃¬ª¦?›4úD
æœ?¢ÐàyRµ?êHUër »?°èzT­®?µ¡$<ͼŒ?£åܐ(ã!?¸,g¡=¢?ªEs60±?ï©Ï{Ɋ?x*ì¢1p?_hþ9=Xð?Z̵SÞ?Ÿqåòz?uddI4FGL J1457.8-4642¿åé*ó7‰s@%©fàé´À:ôé¦ÙÀ<\E–F_@!¡Í­?ÿ_¥'(^?ÃÄÿa©¿¡I÷šÖ°{?ÛÌsvaÑ@ž™ÔÒÖ?ëUë#Ïèá¿àtÜ?,f?I\ÈWó¿Ú×7‰Úõ¿ç@Z˜ÒÊ=?Ðßn"¤AGNbcuPMN J1457-4642?ê©©h}ÂJ?½'Ç=ã™?nߓ¤|EX?a–Ý^ÿ¸ý?ÄÝÜwÂ?½~)|jw?⻢t°¥?˄uå"à?}èµojµ-?Šå°"ž—×?ۂååXóâ?Ë;H´Jts?ë¼½o½rø?¤føƒ•?'(¨+œê?qáHã@*B?¿Ôÿ| Ë?£x¬-œIò?éÍúÎ;?ªÞßÿ?ŠOÍôÈþZ?ËÌ	­Ä?Ê;Ë8¨7/?ªÀÜ1fqÁ4FGL J1458.6+3722?ä:› @N°hÂa9À:@±gìxdÀ<'¤@¼ˆ²@šD7guZ@§À£Éž?¸¦8ŽfàŠ?«ÎoU®2?ñÀgc¼h@
TœåT¿ê7ž&ò¿Ñ¼J^H¿á‡ÿ¨Â+‰¿ä'Ôôó¿Þ@°ÿç¬L¿ë4o©GhAGNbll3FGL J1458.7+3719B3 1456+375?ïá^D+ÂÙ?b"œ'=Í??˜K_
Æ?2Ú¥/_"?j®²h[e?a_]ëä?ï²Ö®üç@?'ŒrÎÞ¬"?@(><¡Íþ?O†>A‡›?'GÐ\üp?ˆÓ¾|0É?ï)Ýj<š'?€íW²khý?q2NNJ4?pŸÛje?–`F$ºÍ0?z½|6?ïÌ8\±–?ag´½?Uã²ûq¤?D7¥ Î#"?t|÷ᘌ?` ¬÷"*N4FGL J1459.0+6129?ì=É9DoF@HÊnÁ~ºñÀ;NéH-–;À<ïóŒT6¹@£À"'Œ@þú¤vln?Ã¥tU·B¿š³ ,Áæ?ÔçñìA[@$»]Ž¦?áú¹¿©Î›¿ã1bV}¿å/áoA¿Ü˜/w便êŸWH¼1t¿ïêøÒU-AGNbcuSDSS J145852.69+612813.8?îåîãWè?šƒ5¶~ @?|è∇UË?z¶1EìS?œ	s-m?˜E¶ò«}?ïAHm]|?"fÈø³î?XªÊ¾Oê?dpzIçRž?–LPÆo`H?'9Zˆ<¢?íÏbH«Ãó?"'́?‡9J–üó"?y\ÛË?­;ˆÏ"ƒõ?ò™Lƒõ?îþCOE?Z˜®©?‹w–®`4©?v]	?'ƒLGý	?x'†QyV~4FGL J1459.0-5353?è‰ù"Á @Ú\ØH+À9½òJ·À;Y^Sô@§ÔNKg‡@Ն¯²
?ºÒ]Ÿ1Lî?Á$xFÜ?ò͗b‡´•@<Yÿ$㺿ïøe˜º?ïû
H5#¿ãší!*È¿êµg £#0¿å$WÞ8Z¿ä"%B{¦AGNbcuAT20G J145935-535047?ì'6HÐ?±-¬ð|Ë?‡Å''¸)?ˆ‡ÒcC•õ?¸}ŸbzÛ?°j
4ê'?ç"4è;?ÇY,Bٕ?ˆꄽÍS?šÁxÏqK?ÑøgpA?Æ£}/BA?ão¹ËåÝf?³ô=ô
?ï?«	Ø]Z?•oÆ_D¯6?Õ½k-(™â?±äQ¤í-?çª	µÏ?¨Ý?=ébÝ?¢áš{‰êª?'x5Ñ)8Œ?̟r‹Hõ?¦ÙIØy¶4FGL J1459.5+1527?痚»ØˆÃ@M
AÝ!êÀ:ÿ@Iœ+DÀ<œÑ*)Ÿ6@*èãXÕ@Â|ò—?É2.3o?¹y}†8ê?ñ%õ'^éš@p½Úìu4¿ê¼$ô?ï‰ñ Á¬¿ÐÏ(œ¬Hž¿Ü^IA<‹L¿êÙ8¶)ó¿ÔvOýï.¡AGNfsrqMG1 J145921+1526?ï>- Z7?ŠRD¯M!*?bm¿–(ÿŽ?]"Šˆ–Y?‡UÒ_2$?ƒžK0Dý?!Ef?ˆô'9g?Feãsô6?Y˜7N~?†t™wg?‡5¦´Ž	3?îIgcH	d?'g–½$k¨?'/?v¬?~€NúxCZ?¦Ýºaæ'?Ž¤ÛX1
?ïŸ~'IÀ?rèy`44~?o§?¯‡?^kjMSÔ?ˆ.P™I¤C?oâª(ž4FGL J1500.7+4752?ëÆGf­è@L¶°hÀ:VL¼q4÷À<Q¶3-Sö@)´½atå@‰‡á
qs?Ä<37
à?ÁƒxǼî?ûúí!*È@|è7"î?áV.	þ‡¿äåܝû(¿âØr‡ÜØ´¿æ- í¶Q¿êÌ_iœý¿ïþ·`Sý®AGNbll3FGL J1500.6+4750TXS 1459+480?ë]KfƒûÕ?²
?¯Ù?¨ùOö'3?£Îp?¸˜ýCäà:?­†sƒh?í{A:ÃÓ?©ëaFmR?'I­o´?"âÄó±
?¯ªÅ,Ҋê?£–¶ò)JÛ?ì]Þz¥µ?ŸÔî_"2?™ÓzˆY%?†¤EŠ?¶Öì-ˆ¼?™LUáhmÔ?éfv	»?¢~80CP#?·A©Rzµ?œÌ丸–?½Š¦?_­<?ž21M¤ëÔ4FGL J1500.9+5528¿Ð+"ÁÐg@J¥éᰉ À:ä¸qËõ6À<¹ªYÛ=©@oœÅóë@qޟ]'ù?Å06(°ù?ÂA!"µ?üê®ñð@#zÉIàt¿ïôL7å?ï¥~ª*
–¿ß—ºò.Ü¿ÜÕR'XàA¿ëó×"f1b¿Ó$e$œíaAGNbllFIRST J150106.2+552750?î¸Eêê02?š)3Ó¯í?ƒcÓ	"	?~u"?§î?ŸEY µ0C?–µQ}½HP?ï۟€þ«?—÷í8Ê|7?iU#zið?uƒ—ò™?™¹ç "
%?"ÓX´§<%?íºÈ1?É*/7¥?"8T£pbÜ?‰kxæì^?²L—^¼?—íàh(?íÙ]nØ]Ç?ú4? õœqú?†ÑUóÆS?¢Z3vu±–?ˆ,(4FGL J1501.0+2238?ïûÚŒ«
@N,ý\·ûÀ9Å㤀À;ýåﳁ¢@úÌx"n?ÿÆ·	)?¨Ì7Tüº?­@
ÿYß<@3Xz™@ÄÓÏöLù?Õcä`è"¿Ûžœ7ً¿Ý©aùDO¿ß¨"í8¿ã
O¿…ç`¿á€`•AGNbll3FGL J1500.9+2238MS 1458.8+2249?ïð ËT´¢?U©ì[ú¢ù?/AAoAÛ?(Õ㳤e1?ZÖA(®'ð?Såb–‹lõ?ïùDøš?ˆ ¼î?L[¨û©¢?Yx"¿Æ?ŠßKô2Œ?†Ôý\Ë?ï) Jœç«?€4}0"XÓ?n
¾b[H«?f'²am?—
>à¡®?|X`¬œ?ï—*HË}
?p,-Ç#ô
?jŸ£öä?VÛp!Ä-?ƒ°…ä#8Ì?k]ó÷"4FGL J1502.5+5552?®‹ëúó"b@Jo…¸QìÀ:_sN¬5~À<}}Ž¡@…×x¢S'@ú <¶i´?¿0'ùD?Ã=ñÓ'é@ 6^`Þg@P±šÂ?ÏݪÀˆpÒ¿Ýz\9â$¿çEb¹2¼¿ãecœ‡Š£¿çªs;`ÿ¿ïüç|{{¡AGNbcu3FGL J1502.2+5553FIRST J150229.0+555204?ï§Pý?
é?{²r¥Ĭ?k—Õv‡6F?h3êÜ>…?~‹–¥5oí?vV60ÃKÐ?¥¬ƒ?ˆ2¹±úèå?P
ì0%ݳ?]œ¸žœÎ'?ŒYڃ?†°4Ž¬7Û?ï&¶:{ò?ü ÷VN?s~ä=™.?dãûèI"?™zÉ¡™?~pÀµ.›(?ïg=yJË?v5÷¢"?y'Jnè&ö?`÷Ò]rƒê?‰œüuëù§?såvPÿ§4FGL J1503.3+1651¿æòƝ¢Ž@Lï9C¬ÅÀ;4<ËbÀ<šáìÂo@ îÐ,Ӟ@Ü¢Ûa»?œ{á¢ÇÁ¿¢Ø€'y©?âU/<-­¸@³ch…$˜?ïÜe@Ìxê¿éÈLŸëÃ2¿æõ=Ïng½¿æ±Ï»"–%?ÁuîÚÛz¿âp· gAGNbllNVSS J150316+165116?î‡ùî$Në?d,Ò_èw?i,2:§•?`;¿Oi&e?¥înZ—fÛ?œ±Îû((Œ?îp×œ™æ?«8îÚ(j?r~J‹Ñ·X?"©Üm!ùo?¦§)4¼*©?¨Ž,˜Rö?í™È'ì'?"ÒnKõ?|/ųsYa?fãbx(?±nÃ9eÞ?'ª¿äÌz™?ìý'Šs
?ŸOse?qÌÉ]Z?oëXnàX?¶ù÷¥©Æ?žÁ. q=?4FGL J1503.5+4759?çý!:Q#@Lx•¿ðExÀ9²amaÚÀ<I핚0˜@ÜB4-@"j㣨ç?²âÚÖ$å=? Èé_Ìæš?ï
	žs`@	4\Ç×­¿áÛÆ«±Ê¿ßێ0¯Ë4¿ä?KâCW¿âyÃ:|Ô¿çhƒweR¿à"¯\y}šAGNbll3FGL J1503.7+4759TXS 1501+481?﹖2­è|?zRF—]S?Tšò¡~­8?`¢ þº^à?~*¬?vW³¥e	â?ï'N–sŽ?Š{~w:Ýò?QÍ«N²3?f¡ëz§Às?2¤ùZF?‡‹—ôWí?ï8‹. ¬+?|ø0 Õ­%?g¶Ö¾V¯{?VÎË	·§?•÷¿d¤¯?z½ìñÍ[¦?ï!<â?!?)ÑÖ`~?…€üȲÂ?r™&ipÂ?'ß^ºÁ?ydYãš
Í4FGL J1503.6-6427¿èI‡‹ÉDÀ"{¦iŒÀ9‡B,Ë:&À;w›9¬Éø@äuÚ͖v@¹NþjԊ?ÀÓbDé?ÁŽe³ãó@
žá×öÌ@
¢¸ý0?ïêž‹¥»?ĶúÓpTý¿é°Oô4ã¿â1i.—ÿïøÛH"?ÛmNâçxAGNbcu3FGL J1503.7-6426AT20G J150350-642539?ì°ÿÉuì??®•}pô m?,µ2ºZJ?Ö
éw#?¸Rk
ùR¸?­âÞríÁ…?èÁ\qc³ä?ÆwnB	Å?eìBM¯'?zUôšO?Ì¢Ý1=
±?Æ9ó±èZ?èì±5–Ñ?«½þÕ?¡peuc²?'ŒÚòÉ2ô?Çñ!ÌNÌÏ?¨ˆãžH®²?ì[\þ®SA?.c~Ûë?‹difw?x=@Øý¼?¹Âµ¾9(?›P(qç'è4FGL J1503.7-1540¿Ñ
)€E8@B?ÿñÀ9GúËã˜ÁÀ;Þª; g@ ~fpâ–?üLû[V?°ˆà <ó?«ƒÛÂ3?þÓðÈT˜@P†èçày?ïáŸØwü¿¼†ˆb¾¿àÐ^¼>¿ÓÙÔ½\¿Ýt§¼òå¿Öyɺɕ
AGNbll3FGL J1503.7-1540RBS 1457?îLcréO–?ªm*3t!?lkµ"è)?p:èﮀÉ?©q²Ø,?¨Ò:£¤@Í?ï&}ñŽJS?–äïì0?hŒ| ¥£?sŒšn–"í?˜¾Þ² È?"¦ ¬(>5?ì҄†ÇȐ?ŸëgV?‡ëhYíó4?xŸžèí>I?¶nn¾ƒý#?[?‹LÈ?éÿáQô;-? ž¨)¢ñ?¢#΃Ïjø?†Ëi»ƒÝJ?Ãw‡;8Ž?ž>h\a¯$4FGL J1503.7-5801?èZOׯ?ݦ‹D—3¹À8%ª]6;üÀ:Dã¼ÓZ†@BÞS\ôM@ÔxþŸ3?³ ~Ôá?ÒL''ØÛ@!€¿®Y?ïî‰ÿó–?íœtà|¬ú¿š¿?#49¿ã§ÿT0¿è%d=—:D¿ëê¹FÞ
ã¿éý¿è,AGNbcu3FGL J1503.5-5801WISE J150334.23-580119.2?o&!uB?eT¸ûqW²?ã<jµv1x?Ê/P¥~‡'?ÙIHю%?Ê$ãֈ?wÙd]:™?€X•Ì¾Ú?àîD-^t?ËJ$Á?ÝÄÏê?Ë	?•dZ¤?x¿µ·€?‰¢4)ëú?ã¨:9??·uW\œïY?Ö×ÿ'Ža?¶Ÿ•ÛýT?Y&=Å
g?C\NRî?ÝܚßÎK§?¸q¶5¢ö?áq6Tø?¸|—Jâ_Ì4FGL J1503.9-4247?ê"!…FÑ@+k{[À:5âÏòÀ;ý+ÐhbÀ@‡[ÿZ>@O¡—Zû?ȅ#ÖH÷k?Ô©Äõgö‰@^n<ô}@ITݧæ¿ïÿýFKê?ïÿÞý¦ßR¿å€èÈ«ÕÜ¿è>¸c­O¿ïþ³íQ¿îv¹?|AÅAGNbcuPMN J1504-4248?åK*ipRå?Ãjg²]˜h?ÆCâÐtÉ?½†Æêœ5?ĵwn?¡?½‹$¬f!?掚:kÎ?Æv8€Ý?Ãà˜%&¦?Áˆ®çŠ7þ?Áäÿr*!?¸S W"ØÊ?ß[ß÷¤{?°'\½f?Ý?Ǩ¬Y`~Î?¤‡nr©?ÕMóX?¬‰­ðŽ±?ãހSÅ¥N?­œÍÎhCØ?ÊåxKE)?¬ýGE7"õ?Å †Ÿž%?¢Ä$°Ræ4FGL J1504.4+1029?Øb˜)_¨@KJ¥ß"9çÀ6Uü6GÀ:ð·E|@á9Q/r‰@þÆDƒ?€OH¬[?¹>àæ_E
@1`m?ž{@#MG0– ¿ÅiÌLtM¿ßzûÿjXä¿ämÂæ™ým¿ägHÐöR¿é:®ƒ¿ëŠ7KšAGNFSRQ3FGL J1504.4+1029PKS 1502+106?îà½-''?˜Ü?zD‰š?o¡ ß=ؾ?r¾*D	E/?Ÿô63È_?—¢nœŽb¯?ìð®Ö^?Ád%GŸÝ?¥]§¡cÏ-?ºð6 ">–?«—jõ–O ?±
-‰Ìtj?îG%¦þøÞ?žàýS¥4?–£Ò¤-xt?'ÏnAe•? ;¼=ùµÞ?•—	®:•?ïkÉò[ã?šžŒ#²UÁ?ƒÜânǏ?‡‡õIüî9?'äŠP¼
?"}áde4FGL J1504.9+2027¿íEeh ¹…@Miáâއ	À:'èYñ
À<q¾7Ô
@•)h¯@¼l}ܟ?º8yÄ<¿£Š~•?åtU!š"{@ñm@U¿æ°,X¿ã8Zðž´¿çu\}ÚKf¿áÕë#Ïèá¿ãކžR¿ïÝ€ÙYAGNbcuNVSS J150503+202811?îìtE~b?˜;‰cï ±?o@›Q,%?c=²©ì̗?ž‡¾
.X?—b×ä-´?ï=¸w![â?—löJ ?VçßÛvÄe?aymA•Êõ?–ÚsU?–q.Òfòí?íüÊæ3Ñ?3v9zÆ?ƒ"¡'$è8?qð9I­y?«R)NCˆÛ?‹mk:ÚKá?î=O+'½?Œê!"=¯?†™Ù;,??t("çïõå?¦"Ëø	?‰|vÉ{4FGL J1505.0-3433?ݕkQ‡²@4°•9¸ˆrÀ: ¤¸±À<;2U½¡·@"¨¢J˜@…êZ|MX?À3ˆX(¶?À êæ`G@<9ҍ×@
†AÏß?Þé;'¦†?ïâӟNå@¿ä~IÏÞ¥¿âX»¸¨Rš¿ç
z!¯'J¿ïÿœb¡µÈAGNbll3FGL J1505.0-3432PMN J1505-3432?ïܛ·­š?d}
'‹M9?ZÉ4µŠÜ
?TÛ>Ëw²?eÿ­÷ y±?]©†_1.A?ïŸM¨%äJ?…•="9‡õ?RP¹Pҟv?d°5®ri?…â~Ìl™~?ƒYna0°?îúW$î?'ïshñÚë?ul6Ðü\?gµ@ORa?›bǓÇÂâ?€Cý".W?ïôÚô8Ÿ?€ÅÉ;ö@+?…ø~ÛÇñ6?rØꕫò?"%%3"ó‡?wšÁdÞ4FGL J1505.0+0326¿ãÐù=@I!lœ
"À8Ó§óÏpÀ;ìнU¡@;Ò2¸@ê¬azŠ?©ˆa97??¹^èî–v$@`dÄ¥¶Þ@/½É¤¤:¿Ð"h<ªUT¿ãµ´ÂêÌ¿è1¤½º
R¿èšc"åV¿éœ¦š3¿ïÿrܖnlAGNNLSY13FGL J1505.1+0326PKS 1502+036?ïːæO¡[?t¯Ñk4Q?^³ð'¤äê?]3€ùŽÇ?rŠ³Æ?oss›—]?ï~jÉF?š‹`­-"?i^m-ˆ¹4?}1c^'Éþ?šÒ¢ŒõÀ/?—àª	Á?ïg÷Ն?‰‡Ãkz?tâÇr,?mF½ˆõ]o?šzO(«tâ?†ïØàáŽ?ï…'k{?t±"fÏÿ?ym+æ¿Ø¿?hÂ
û²ØÐ?')Å4²?käºÔ¦ÉW4FGL J1505.5-8241?éÆO?Ù4À4ú9櫛$À:¡Ñ'¥`wÀ<}kgW'.@ >K¶··'?ÿ¤;~[O²?Âsýiw¾?©/†DA\?é«ù®ro@ïÒÇÄ?Ä4<»Ív?Ë*ž¤›U[¿Ó=Ž >¹Ï¿äXý'«Æ¿Ó˜úìð¯¿ä*[…~AGNbcu3FGL J1504.5-8242WISEA J150525.41-824231.1?î—ZE	‡‡?˜ä^ê'?pñ$ǜ?efïÒG'¬?¤ˆùQBî'?—¹9ŽNO}?ïˆ÷1"Â?ˆhTÒ·aä?@¡Züž*-?Sµc#`‹?Œ¸Q-?‡'ô‹¤Ê?í¼uOÔZ?'rKŽ9?}¾|oûe?p\|]æE?°K陖/t?»àOÖ?î•Ðßð…?†íF¸Ž{?q4÷rÔÄ/?`~}JúÕº?¤‰$¦_:?†â–3 q4FGL J1506.1+3731?غ"µj@Mó'=[«"À8nd"ÕÀ<3mÖQ@D`%Z@/Þ|·â?Ÿ'†yù—?ºA–{@GՁ§4@Ÿ¶'³y¿§¯Þ™AÊ¿ãÑél?Ä;¿çO'ðßь¿ç¤8#\üZ¿ë=8À:î¿ïþ½	á*RAGNfsrq3FGL J1506.1+3728B2 1504+37?'1¾Å?'Õ³)¤ü?v|H±qW?C¼sÀ8?ƒ·[?ˆk‡Z³Ç˜?ï]҆K€?˜Íx$[?\ßJ-o}?pUP"Wê?'wºšhç?–ÙÖlYÕ?î³[ð*L?šßM—H×j?'çjÙP?€!QRTî? lj¼×«?˜²§$?ïú7;¥ÇÜ?:ÒõÄ¥?1$()á?'¥óÜèf?=!ú¨¨"?4ü]I 4FGL J1506.4-0540?á\˜o"!¾@Eܺ`À;{kà"êçÀ<ž`·Ð¼@"ìr'9Õº?øYÙû‰xº?×\ýç!?Ë©=¦~¯?ñÉa=1¹¶@/ªÁŠ$¿ï')` §¿ïéMcÓ?ï÷3¨£ø˜¿×§amÙ!o¿Ç<ú\Rn¿Ó^U`Y±øAGNbllNVSS J150637-054006?ï—¿"äð?š|¤7º?]9ÝkPl?VŠ4¬'`?›Ùj6Î`?™³Ñ¹UÍù?îå<'Mñ?£_[v¼yÝ?f'½äc?{êý?.²õ? Jô¯B¤?¡ºnÅâ¦?íWŒ(>?šh½ÛÄê?{kÓ¯\e??qFܦ‡†?³ŒÞ»É‡¼?™5‹øCø?ìY4s±n?¥Ì9Á÷?OMò'SÑv?QfRô?¼÷À'GÌò?¥»|ÍNð®4FGL J1506.4+4331¿éøxÞI]@M!ý`éNäÀ;CEћh§À<˜&B‰èL@xU'¾·@¶ŽYÊv±?ÃٙycCF¿§‡¾د?äöóaŒ@ö^KdØG¿Éà ¢6÷?îÁÿiW2¿âg`âC±¿å‹	H~¿â3''d3¿Ü™špY.oAGNbll3FGL J1506.3+4332NVSS J150617+433413?ï]N3aÄ?'1¼ÏåH?xœÏî1OY?q]pì¦L?–­">sà?Ñh‹‰D2?ïu\ÄB±?Œn´<¸<?PDêf´š?^Ôê·»\?P-Ái	?ŠrÐÖÿ6z?íšÂ#_¯?•P‡gf?…8DZËä?t,#&†U?°‡‡Üw.€?'—'ÿUtÂ?EÎi¸?Š98M—?'i¾+ŽþÏ?w{Õm؜?¢ºü5¤Ú?‡ruÛp4FGL J1506.6+0813¿èvKŠ±¹@Jl÷ µíÀ9_N"¢Â7À;ÍßgDX@¯T§¢ò?ùŽ%)/?³¥µ%ç?¼<©>'X	@—ƒ>äA^@Û¯fœA¿Ü]ÝÙ¥¿¿…	ꏀf¿ÓþuÜ{ ¿Ô!}Uì¿Ý²ú"¯tÍ¿ÜÞì>Ø
AGNbll3FGL J1506.6+0811PMN J1506+0814?ïä€ô¡R?o]¯~M?B"v??•rìJÓE?fùæZŽ
²?lš¦ñÍE
?ïs«Ý¼=Ì?.e=Ú?S"}©¼¤?`ðt^gç?R<mæʌ?!îàكV?ïˆ*÷?'çÙºË?r)%0*)?e'"›R¸?™Dµ!ðó?‹Øxk±P?í(õÑþ¿?ž.äðk?sòrq§›P?`/Øýg?µy*Hïj?ž.i"'®04FGL J1507.2+1721¿æ½«Oà¤+@L™£!h0À:‰\qÀ<Wκã–=@ em¿öûu?ø‰Þ¦$ ?Ä/g Ë}?Îæ|¡;N‹@¹A|¢@	ت•yµ¿ï~Å`?ïp?}ÄPý¿©×!~CÁ¿×ŸlAqºW¿Ò`½§?õ¿ç"T¼÷AGNbll3FGL J1507.4+1725NVSS J150716+172103?ïƒÙŒ•¥?­7ú'¶m?~þt¦nK?­4Ó­Yû?€	À‡_}?y€âêWѶ?ï‰Ôþwwí?Š‡'`­";?Năۅ+?^Ù½2¥%Ž?‹žx$i±Ü?ˆkN	á‰x?íÙ`ñ¾•?™)™É'ç?'´<¬"¦?‡ÞBìÿû?¯Kššg?"vªr&?î%²'m¸Ã?'£J
Ì?r"®vÅÎ?e½Y—'Ê?«bŒóUšö?'X`È_N4FGL J1507.3-3710¿àçTñQš@25ƒƒ­Ÿ
À:_'j@À<L$s|Ï^@̤.Èë@wÖޞ†h?ÂXê§Ôó?ÁG֘Óv	?ýœ¹ßŠ?@W?Ñ&MÈ¿ïÉU^?±?íf.¢<Ö¿è]œ"I¿ÚébÖ#c¿ä%ßøù{'¿ïÿï¿@PAGNbcu3FGL J1507.6-3710NVSS J150720-370903?ï2Š-)ø¯?¿$«äÛâ?ƒ"A‹b#?/æ•9¼?™•á*?"±õñãt'?îÈ*Ó÷®´?žÃâc*&ë?z5!Ds'?"—ÏÒÞ? 6¡\†S?˜:¼2 N³?í@"^T¡œ?—ãxìý?ø{³¢P?z© O°?²[­ýä~ß?"]'=Uä¬?ì3ÛT4k<?•f×ðÕvZ?¥jŠbçª?Œ§oôõô?³«àQ«2D?3ì«°$©4FGL J1507.3+3341¿êÏú#G-@N·=CÀ;1@À<Ïâù^ü@  ¿þˆ1?ø¸¨RšÈ?Ó­Ü|m8è?Öõ·ý‡Õ¢@f݄ªõ@\[J©q¿ìiþ Õ®¿ïæ»@2u?ï›r·­¿×@>Æå,¿áp¿ïÿ⾦™\AGNbcu87GB 150531.0+334938?î÷'È'B®?¡ƒ1nÇ£Z?pÓn¿CŠŒ?u!ãVÀïÎ?œØË>Ǎ? VÐóÏÙþ?înEC6W'?°N‡kÛz?qUeHT=?t`!"¸?¦ðÿ±|a?¯É§èq¥	?쀄¦RrË? É™jN+Ê?Ž°£¼Üó?€+dkKA?¸%Ù8ôÍý?¿k§$;U?íYX[-ƒÈ? ž–ÁŒt?s7É<¢R?qÚìró°?´™ªŠ?Ÿ¸³'»4FGL J1508.4+7717?ätjžbç@B¬ÜY1ÊÀ:ò¦WíýŸÀ<ã™hò1á@c`í*»@,næg¨†?·ž¹¾þ$¿µÑž~ìÖ>?úáՍe®±@‹Í(<_¿ÔǙœž±±¿èï^¶¿â—À%çñ¿áž2OÞd¥¿áüE°ä9¿Ó9ïô8AGNbcuNVSS J150811+771819?ïʃ·ýý?}zæwäà?S­³<±*6?OŸ}'?uÒ·iÔ·œ?{Fßò?ï³ûå?å#žpÚ?@ošªê¯ï?R	"<?'8ƒU[ç?€Üxœ×п?îñM{`o(?‹¿ý"®Ø¨?gËzµ%?g€ÒâT?žÝß$›vL?ŠnÅo'<¸?ï½õ!°ƒ?iÉpÉl?Tàºújá?EÆWEŸê"?{Í@ ÿÖQ?iL£@ü†M4FGL J1508.5-4951¿åã~JïΖ@Ò´|lbÀ8´"}Ðæ7À;; 'oÿl@œY®ê@žÚH¶R?²5Iè‹o?Ō¨Å["P@sœcxu@–,ÞZi?Ø¢@\;•,¿æNI¿ê5`Iô¿éF3 ÁV!¿î 2:ïÿóÖ&ãAGNbcu3FGL J1508.7-4956PMN J1508-4953?îÓC³À(\? ÔíÃÄ?™}ׂ»«?›úÔ¿Uê?ˆ3d
ºqh?"‰ÿˆ¡…!?ã×8/`ô?ϧ'BÃWQ?ÂۓB2´?Åø`Ü"?А‡î‡ä?ÇÞ/×;C=?뗠kµÔf?§P6 ,?©CPˆ¿ûW?šEYD1Þ.?¶¡T]ñ_%? Så	«?áævZSÍõ?®òeÝLL»?Æîô©q&O?ª"™f5–ú?л˜öŸÐð?¨ã7¦Ú{ò4FGL J1508.8+2708¿ï´š	/@MÄ6~ANÀ: $-ÿîÀ<Rv‰Ê@~ÄN##œ@¦M™æÆs?ºâL¤>Ó¿¢F—'×Ïú?èŽÙ·–Ú¢@5ù¥ž?ïìh ¤Ñ¿ÙãºÚ±çÄ¿åëÍ
dl'¿àSÞ9ۿׯ͸…,¿Ôá,Ö!à%AGNbll3FGL J1508.6+2709RBS 1467?îéf""W?"¤1§Â`?m;KfÝ´?`†Ý#<H½?Ÿ+ÖB'¾²?'¯f¬.ug?î؄'à?™_çÎîŸ?fó%8j!Ù?qû›¦ë*Ë?¡,6ßð?—{ÏEªQ?íÁhfL°'?'ِsKêµ?9֝d™'?lxÙC
W?°cÄ1×?'[ž$Á<Ÿ?ì»®ÎM¢?"Ë^I·?"DIý׬?'ÌõŒ•:_?µw'î?"'ëUª¸Ç4FGL J1509.6-4334?Ý'å—"@)Íl.ýDÀ:êHޖ#À;á•ÊØ@Èý4s¥@¡íý¬i?Ë|,Ñð"?à.Ò`Š"S@})Àµ@n埬ƒ?ï¥(xÅ
¼¿â¤9/Ìvf¿é½¿ÚËé¿é×ñ=Å]m¿ïÿù_|è3?ïg4ø/Q&AGNfsrq2FGL J1508.9-4342PMN J1509-4340?ÞÖé¿Rä?ÈDã@ez?Ý÷ºW?ÉzûÓFžÈ?©ŠáUe8°?¥â3%Š¥ñ?Óü™OâÁ?Ë0O¶if?Þ¦×?é?ÎõŒ$єô?ʹ2MŽZ?Ä+¬Õ> '?Ù!½‡UD?°ä‹ÅËò?Ò1ñoª¥¶?°©ZÕëçr?Ô¬QŽÎ?­¢zÇÓC?Ë«M'|?¯'fŠ<ùõ?àyR6F?¹áŒÖ·?Ñ8)5µ?³£vüu
4FGL J1509.7+5556¿çÆÔ\°|@Jo~=ÁÀ:@K!JÓÀ<ŽævÁþ=@ 0@	‹€?û÷.?½iSWjö?ÀD,?Nœ@Z'£S&?üöèˆ?)?î0Sà&ñ±¿æ·'I%E¿Ý2;;•Wk¿Ñ¸䓒ï¿àñ¥"yŸ(¿ë'ž^ÿëAGNbll3FGL J1509.7+5556SBS 1508+561?ïIgM÷²¤?…Ÿr¥FÏ?qZü`x¸O?hÔܼ'"?'|W(ë}P?ƒ
a·›?ìX9š¨F?µa¤•áÜ? 
¨ç"/²?¦rË)œ?µ8Þ»±¥ò?®sæà˜A?í­Ú…`lÍ?"Êá'opŒ?""|(/ô?uIW÷Þ?°œQ7""?'XsÏ9Âb?ç"³Á¬@Ø?¥|ÁpÓu?¸¹ì0wXŠ?žÒŸ"ÿͯ?Ç:áP\?¡5¨"ÒêG4FGL J1509.8-2906¿ïÏ_·
¸@8¹yŠ˜À9'[4<ËÀ;ùÙLJ®@Rü'G—@3n<½€?¸'Þ½?ÁÇp×ÙpI@Š.oKè@®w!I§¿¨ëÂlÕ¿çòÖKÒ¿é0]€c½•¿èœPbîâ¡¿ía¬ÃB
¿ïö¾7ޓŸAGNbcuAT20G J150945-290502?ïÁ‰ƒoê?z'Áâ
'ž?m²VW?n¾kŠ¯?p¸¾eß°?n™ãN9}?ï<"º}¹A?—o@?f£¦m/+?sý}×Ã.?•§3â—1æ?•amþÚN?î톌rÇø?‡.¥r
`?|íGþ'8?q%Rð?›Ür@Y?'¼íoE?îжç=ìr?"2Ý ¼?†6©>H?p»À͟?šÍÎyjP?€ím¨u4FGL J1510.1+5702?àÕt@IªB¿˜0äÀ:¢<g[RÀ<ª4òP@¸ˆå—I@
4˜?½€žöЬU?fmȁúƤ?¨á߯\Ï@ú8õêÓ?å4ªÌÇÄO¿çvÇý°Ž¿ìܽ¹‰y¿å/hۋ¬¿än,Rn¿ïúÎg×®AGNfsrqGB 1508+5714?ïT¥™?dK_'1ù{?[!ÐRǀ4?bæ·TD
²?6ªìµ4F?;Ì¥¶}?ïxUrþÑ?'t@úø¡?M·¢—Õg?a¦TY$!Ç?ÆzÎb?8@ÓxšL?îÿ›
³M?‡Æõ¦õìM?kÇwK"T?dôDZcõ?œ"Ÿ57Ð?†"G¦òo?ïÁãCót*?e)7Ö5r?iâl?Z—áHª–?rS½µá?\ÀSaHSŒ4FGL J1510.8+7959¿î¶ª'í…@A•¥CñÇXÀ:ßB¶]õÀ<êž…@¿kÅöÅ@Eʯ¼Î?Â(Cg2ê?«
jØf?çù4j¤9@êÓ_Ž¿ç4yð'Î?ïî6¿Yǝ¿çD{û#!m¿Û§˜€|¿â«5£OûÁ¿ìïÐ!ëãAGNbcu3FGL J1512.3+80051RXS J151026.3+795946?îÛó™?k?¿–˜Mà6?xÄÔô!XÔ?–'NcSœ°?žPWŸ¯¼O?º˜ø®õ¨?ïÁPi¿Ñ?~ÒvƒÖÜ?:£ÃÉV?PÏ©Y0)?}·pã'[?|ó¨­×?ïa×ú/?‰!¦íJFü?jÓZhìñ7?k;E{]É¥?›™YÒ?‡¿AñHç?ïò*há?FvS'-?9ŒSí²n??*ŠÜî—?UHâÑ'y?CŸU闉þ4FGL J1510.8-0542¿ÝLMn@Eyùa€M˜À8ؔqÌÀ;"
ɇï@["Ì´@71½è?©°åæyF=?¼¼"Ûw4•@YyámmÂ@P¡ú'+6?–ž=¿Ò¨˜Â¿åÇ#ªÿók¿ç;,%ø¸
¿ê¨¿;ê'Ú¿ãkÀx*´	AGNfsrq3FGL J1510.9-0542PKS 1508-05?îg®þ6Á¥?±FHnBÖ?n€CÁ£ý?kû‰^Í(?§ày¥È?°Ó5,R}`?î¨ÉþÜã0? 2®%lP®?wôêê8Ò?"ÏRøo?¢t´겮?›/b"–0Š?íbñôÄþ?¡'X—Ì»?˜M#Q;݁?Ž>gúi'?±áŸœ
à¡?šáEv­À?ìÉý>ý0?•þ¾¹q)à?¢VÜFqÝÈ?‰QV_ ªÈ?°"§ç×'?#L²Õ4FGL J1511.8-0513¿í¤u4='@E[|þX`À9‡ž ç×À;ò鳍a@ ‡øø#è'?þR@ßÄ V?¼FHcÆùÏ?¨ã^^°¦?íé"89,q@ŸâÈÇ߿Մ'!W¶¿è¥žTê= ¿æ\º:¿Ç᝿C!h¿áà¥â}8:¿Ú}çAB?–AGNbll3FGL J1511.8-0513NVSS J151148-051345?ïűT'M?Š»X	Û?cçÛRfÝX?VhPu?›
Nk ڞ?‰YPÂõ?ï–?¶Ã;?—dÌXg?diõLP?m1ª$†±?›?ù_¦5ç?•oŽÜ¡¾?ì"±ÃoD?¡~קËq$?îšrq&?€ã¢y2Ò?»3CÕHEœ?Ÿc
'?;?êUG<?¥Ó9ñ¦Êß?•ñœÍê_ž?ƒËÎ7&±?Ãì¯vC­?¤Ñ™™žéš4FGL J1512.1-2255?ÖWÄû>@=~"î9.À9ÎޑoÀ<!שŸ¡@ 	øF£'?ýü}ÿà?¹‡5híJ?³ŠJq=Yþ?ûmAfҜð?ü=aèRdQ¿ÜŸ9`ô·w¿Ô¿eÛüëy¿åtïËÕV¿Ó'vû	 :¿Ûî›ÿzt¿çǸƅŠïAGNbll3FGL J1512.2-22551RXS J151213.1-225515?îÇüT¨Äü?'Þäð< Ø?sÎJË99
?eÖOdÿ?¡q\‰#?'Ǎ™?î`U\Ðą?¤â5Ù»?'ôÏÆΦ¸?‹úê «x[?¥=vA@?žè–#i*?ìø¸:Õº?š<ûKÃv?ŽWé<š˜"?€¨V¹{ߦ?´t=•ÿ?–¬#üpž†?éw~â'¡?¡W|c<ºØ?¦À"Þr…?'Î÷(Œ‹?Äqß?þÀ8?F1б±!4FGL J1512.2+4704¿ï6×<½J¤@L>}QÀ;6©ðÿ±üÀ<äæíàBË@.KAò¿@\Ôí,¿?ÑqD:íg?³#uÐ玚?ãŒf«/Ä@E<O'²¿àdy¡*]¿æˌ%<Ðk¿æ¦j±N¿ÔyK%BY¿àÐI ]¿ïÿç@ìYZAGNbcuB3 1510+472?ï±WÍ?Ú±?}"Ãù¤ì?A•Dž,?7ª'Rªã?'»/µ
	?|iRµ=d?ï€]… ^:?î(¦,?B ½Cê?P˜ÍS0N#?ŽÇ"ÌO?'ܧhOé?îGwW¡ƒû?'jPèÁ§m?q²"•%4?d©BØÚÌ?©RF3õ¡?lº"ju?ïX8ü™¼"?zÀ'퐉A?ZŸµ¯âÇi?M±Â``q?"NåÊC#?zG¢KíÅM4FGL J1512.2+0202¿æOâiÓ>'@Gý›#ÝTÚÀ8Öu£KÜÀ;ɑÆf>@ÁX';§ ?ÿ~Ö|¨È?ªˆSöø'?Ä'q¤€¨@#'\´5ý@SOÄ +¿Ùw<!™X¿×Du»Cš¿àþ‹ Z›¿â¬×cÿƒÙ¿é']ýa?5¿év%@OvAGNfsrq3FGL J1512.2+0202PKS 1509+022?í§¿Ò/|?±{C|åÁè?";IûSž? ˜¯äƒ`?¦Áå8
•à?¦øÛ4û¹?é6€/'Ù?Ƴ·½O7Ã?º'Ûû3Ƚ?ÀPCˆá<ò?»¹"‹úø}?·]Š›NôÂ?êó]øTz²?¬ÂËLy?µÏÆàŸû?£¸ü"œ"?²•J9{Š"?¡/¡Eà®z?å¯Ç5CÑ?¬ŸU™¹þ?¿›'ñ±Ž(?£7ÜÝø_D?És2Ù¨?§uŸŒã6Í4FGL J1512.8-0906?êí&=κ@DËÑ$JbÀ5˜A‰7KÇÀ:k' ÿT	@VP"&ë§@òa|ÚQ?ƒÍ#Ç?¬ƒÖAsE{@'ö«ÿÍ«@!`&	ÿËÄØâ"Äö¿â'\f2d¿æÉÁ/á¿åŲÍÈ¿è2­œ…Ý$¿æð _ñØAGNFSRQ3FGL J1512.8-0906PKS 1510-089?íKú9`Òv?± gÔ}b?r	í4Í,ó?'˜îÃ`?´a¬™…?±áUuƒ?î1Ñš?°ÃLv
̤?‰…Õ:8yv?ŸO-`ÇÂ$?¦"¸ô`Çö?ªÓ"¶Ýp?ëq@eR?¬ð¶ËBÿ¼?"$c^ª[?¶‡NÒ]ê?¾Ë]%*Ï·?«a¨
­äñ?ï.8%d§?'^þ7[°v?\*[È$?ƒÔXQñ¹?'Šô¦%‡8?Œ¸s6è64FGL J1512.9-5639?ߐĀD€Z?ðg¡á^TÀ8Ç£è_ÐÀ:ùҍ.#@T͆=,@dÆS6?´Œ4қ?ÇSy9QÛ?@àþ}=C@ÂÌ«êª?ïÿp\‰n¿Ð
,"óŸõ¿ã¤"CÆÿ-¿ß.ß[Å£Ž¿çIú?KÅP¿é·}z"AGNbcu3FGL J1512.8-5639PMN J1512-5640?îV—Ŭ€b?£dWRúÌ?uã¼›Q3?u W–^s?§Ú"í¤¶?¢>$¿\½?é1l%TTæ?ÊÓ"ïgÇN?läõ¬T?Œ	% PLS?ÊÆ¿R×û?ÊÏí­1Öª?æ¥ÕfŸ´?°êýkÂ]·?¬
9ùÆ?˜‡€SŸÇ?Îe[ç¨??¯ù‰Cž:?èÓv@|"?®íÕz{T?‡Îß÷¦?v}i_BÎ?Ë5Eqôþ8?­‡Úd½²[4FGL J1513.2-7131?íg¸$búÀ'c"ÀÀ:´Ôˆ'ñÀ<Wi¯Çˆ@"y¦	>˜@š"ÛÍÐ?Ä<yX¦?ÎcÜwµ@	£1…´	‡@«	¼Ad¿Ð(³"í?ïþ'ö ¿ãotâ«}¿àhþ&,"¿éU¯"­¡Ž¿ïÿÊñ*z'AGNbcuPMN J1512-7131?ïÊKÓ;Ö¤?"œš÷Î˱?m0ғ䳩?}¸ˆÒ4à-?hƒZ0D§i?‰&f4ü5ÿ?ï¯q¦õzm?"Åz¬± ?9†XåŽ?a?+˚Lú?ƒWŠFÁ?"T»Â1 Í?í5k'ÒÓi? 0Ðïi‰?—ññõ3¦?µÊ+H´Š?°XCDìÅ?˜ûþ¶U?ï¶es€Ç}?k"+Óü?VÝ/Óñ»?IqA‡>3
?úJ؄ù?hmÖÓÿ>+4FGL J1513.4-3721?Ú '¹¨@1h²ú"¯uÀ:b寺À<O)1Q±£@"®ˆ"
¿@˜säÔ*?¿ÊgþÓw?­¼³Ïû«?ñÞ¦éä5?ûŸ5åÀ¿ïo.áêÁ*?ïì¢À‰Èk¿å»àì>'¿àð™Ã¿ÞËrÅz%¿àpÊ"M‡ÈAGNbcu3FGL J1513.3-37192MASS J15131867-3720114?îú¦¥úm?'|H™éX?p§b	üXù?c-=ú˜´h?œ"r¨Áœ
?'´È)óV"?îÆÀ–­©ø?žZ—ß%?sãµ]…¤?;f 57?¡–y¯Ú?™HÞµ&«'?í}Ÿ?Ü5+?"M³_Hñd?…¡äX´ Ä?sLôK?±^ÉvҒ?'0dH¹»?ëە&Lº/?—rmñ1SM?¢ñü-Þû?Œ¡¶§mï?·ªX¶ª±	?"úŒ˜ ¿s4FGL J1513.4-0753?é<–OHxÑ@DuáC|V"À;bˆRIxðÀ<‡çQ³Pû@"/c¤• 8?û§+y*Ž?Ò=ðüVþ?±b;^zߚ?ßÈ*[sCD?ö-.vàÜú¿ëBĀx
~?ߧnƒì3D¿ç+m´Z濾9HËö¹¿ïê[ãU¥?ï²Ã×ZÅHAGNbllNVSS J151324-075450?ïœ@ÅýÈÎ?"_ž&,Ì0?AÇ8n?AæÀ ìØO?‡Ó]mkN?ƒî|ÿ'ú7?íQ˜Šƒ½?±®×-ŒN9?1´žª	š?ŸííG'2Ï?®(¿o?ª	ãv?ìßÜøÐ?œÞFƒR+?–xpÒMÜ?#ˆ(3Mq?µTŠ
$÷Í?šäDôiÜ?ç	pҎª!?¶;›5}?¤i¨?£d`áËÖ?ÎÔbpb'?µŠCÜ=Ža4FGL J1513.4-3231¿¹O•[ÊÀ©@5r›ÏÔ¿
À9v)a"YÇÀ;¼GÜ7£Û@ÛQv?Lq@á#ôÑÏ?µÀÈ\¥?Á•T{ç@ Öoþ@û0$
 j¿×9Fr«G¿åSFÎñj;¿ä›Âhż7¿çè0Àè#¿é{'{;
¿ïÿû˜'2AGNfsrq3FGL J1513.5-3233PKS 1510-324?ï×y8Θx?iǃŸ?Tµˆo)Š?N&FTÀXU?n,0/ó˜?fý,/uk?ﲿ55?ƒ‡XÿšÙ¥?B÷˜‡.$?Zÿ,Äx?' ÀêA6P?'-³S/?îÔÖó­Ð?‹ƒñ<ýv?ªŒ~·c¸?wÞ4‹€.,?z™ÁÜlõ?…üVài
?ïpöLƁ(?v/ë%?U˜\À¼B[?BÓa/JÚ?‡°›$Á?uo³Î<Ôå4FGL J1514.4-7719¿íu#2¥À0¥Ì·ÔDÀ;ǀ¾/À<àÔfõŸ@"á%T"l?ú)'jÑ/2?Ñ°Ëdlç	?Ħ–—±?ó¥@Ìxé÷@åÕÑ-Yª?ÉðXC=—¿ïÃh4œ¿¿?ïëÇkcü?ÛCå½´€ü¿îHFøã?獨eÓAGNbcu1RXS J151448.8-772249?ïfìõ6Ú?vÞ$öŽ«?X¿¹Sår?U-Å8l?' Å]'No?ŽDÕ¡ä‹?î˜õxUš?´ï™(>l–?`ž"}å)?yZ¶sC?¥f¿2ɳÛ?´wºö«)­?íu¤£Lœ<?"ã˜dd?†?©ª´?~ÄÂû:ˆ?±ŠåÄÝI?'Ú"8x?ìüÃãeR?§Vg`
?p¶óJz?ql*½¯*?·q°5?¦'ŸCÁk]4FGL J1514.6-2044¿ïÒ÷ޕÄo@>å.rÚ0À:uÜ£¥§À<Ný&g@ìF±ë@ ¿þˆ1?Ã)Wɱ?³Ÿ™/Ò?ñ*¸¾«¢@25¯O>?ïÿŒÝÉtS¿ÝÀÆCÆ©G¿á$gRõpZ¿ãšÍv?ø¿ä;_‡O:¿â"«äøêAGNbcuPMN J1514-2043?îïóšOgI?¯d-L™ãÚ?VPí[<U?Ml÷Fþˆ? NE[ž±š?¯ZtÍÚLê?ïU	'ês?‹1{ÿLɂ?T™›R+z?^V"¸u@k?"AMš%?‰"-nc?îq€Tå?ððöK-?t"žßíõ?cw"z"Œå?¦U—½Ò€j?‹µÆ#?íÁÙ?Ša?‹uF¡]
a?<*?U)±?d"' '©?¯úæƜ´¾?Š}f8>y4FGL J1514.7-3617?îuMÒpУ@2)•þÚfÀ9ñâ,°b3À<ßMØÐç@1gIp@e›Ã?…Q?¹ì6Ÿþ8?Ï›À:m9@;òá3Œ@©›''3?ïàÏ6iI¿ÝóæÐ_~¿ã9 ²ýï¿æTF›œS¿êjáj)¿ïûÊYêWAGNbcu3FGL J1514.8-3623PMN J1514-3617?î3Q¸gm??°&®h´|ã?£§ì
Ç,?§Ç›@"+¥?'Eðׄ!³?•óñsÍ"?î÷ßg̪Ö?œÞR]©¬o?v$@®¯ºF?'Cá
 Ÿ?›{Ú¾¶È?™h§‰ÿ­"?êRI…ç#G?­E¹kF?¸":rdzb?¥$Û"$õw?´Ùy]ÿ2c?,Pƒ,£ô?ìïcáxØ$?•§ Å؂K? · {¨›A?†½–ºe'Š?°)¶dñC?':*¸4FGL J1514.8-4748?íÑ]'ì³@ Ü˞Ïc€À8ñOäCá×À;y´{/P@ÔT¥sÂo@M/ãóYÿ?­á©þ–žh?º">eìC
@
~BZîc @xŽëád?Ýw€À政â,'à°«¿äS0¿äÕð'3¡m¿èÄ]'"ƒ¹¿ç ¿B Ž€AGNfsrq3FGL J1514.5-4750PMN J1514-4748?ëÔ¦'Ç?¶q"$Ô?k>Î~Ñý?e'IÚKƒy?À@l«ºÜL?µÈ҄Öa?îkÑÞ};z?­ìáåٜ·?\¥jõŸô|?oyég¢?¨]¶ÀHÆ?­ž
Î('?íÚËdzî?–«½ >Uø?ƒÚy"Ùª÷?uÖP@²=Ú?­\«Sav\?"­(†)õ?íם鼩¶?Ž¬PU?"åÚES'?l*Œ|Ëà?­LªÒàš¹?‹Ç!³œ
4FGL J1514.8-0949?è*ßã¼@C¢õ˜ñÀ8äŸM7ÁÀ;;Ò\XÆk@RgÈOƒ@aC?º"ÄÐÿâN?Ä?ðEwÙU@(»ÆKç@ƒá…Ói¿é¥Ï½—ûŠ¿äžæ.CŠ¿ã؎¡îÒ±¿ãÇÏ7
XI¿è˜Ï¤îar¿ê2ßP]¦AGNbcuPMN J1514-0948?ïȟ±b¢¤?sĘ©Ý?XÞ!ɪŒ?Xë»kÔTG?u¨ïÆ<Cz?o¬^õ>"Á?例a›Ö?3©ƒyâ<?B ŠGèî¹?Tì8yÂé?…0žô‹éB?ÔA¶1pž?ì՘`q»G?¡€¢"'?ÞV@ih?†:ŸKµªË?µ§lWâæ?žù8q'e3?ï?ê˜@n"?…Wi´Ý8?Nnx_%¯?Byq,pn)?—<Ô/6?"ÝÑö8ò4FGL J1516.1+4351¿ïi.¤S@L?ނ׶5À:ÉOµò–À<iàš	+"@É´¨"²z?üO§r 0?àxïÕæQ?ægë×TL?ý`« ªšs@…çë·¹¿ë~ê÷Z?¿äöHñá¿áº cÏ¿èΦ´4P¿ïÿšêÒqQ?ïú6È)¨AGNbll87GB 151444.4+440102?ïE™¬']?™a÷P¶¦÷?iґ‡?lªc«éÛ?"%Zª=Óà?—öÄûõ²ƒ?íyÍ¥…à ?¹Xÿ·ÑØ?‹¥åX;ž?Ÿ"ŠoÙc?°Á^&ߌ?µ¿€ÌÜÝ=?ëqÀÃú•?¡ðӀþh?¤™|"ì{?'«¨è@Ï?º)²ûε?`Ø´}?íþH½Iʲ?¨Ÿ±ÌÊ?eÁcÄ¥J?eòÝmèŠ?®¿]óG
€?"n›‹4FGL J1516.5+0015?Épxg^¢¼@G}$
=À:$í`Á
øÀ<6ðÊØÖÆ@ª4†O@ßöZdÐd?ÀFý•lŽI?²À´æ| b?ñ §". @ÄÓ6Hfv?ïÿÿÊPË¿ã»l‡è—.¿æ‡Í‰‹.¿êT
¾ÊÖ}¿è'vYùpš¿ïýHàÄ{pAGNrdgPKS 1514+00?ïo)Æy?"¡"D?dQï%?odš¡Ï?:+/I%×?¦"öÎt?îýî{?•‡Ã<ÃK?e/󊋀?lÿËåþ2L?«÷C¿JÄ?"æ!ȯê?í«|Ô`éâ?™–­?†¡(/0ZD?x΋<‰?¯Ÿè®%KN?•yÉNsŒ5?í¼"ŽPf½?ê1+#ãÍ?˜›é£™?°?€Ë°×èú-?§èÂI,ôc?‡+ìê±W4FGL J1516.8+2918?š7‰üGÙ@M©'Dé>À:Òwú øÀ<‡Ó*´ßp@ò_­Ád@¯œ'r^?¾` |È念Ëœ¡
ý?÷ÑÓíR~R@?¾VèD?ã	Ñäç¡¿ÝQò;_¿èÝ۝ ~¿âfÚ_\†ê¿ïátú}à?ïw¹_‡¤úAGNbllRGB J1516+293?îß=˜'óµ?ž˜ÕºÙ9¼?†e†»îK?ƒÖÌ:Ë?˜åÃ*C'9?˜3)bà+³?îÂOrýñk? 0Áʤˆ"?p,ÈvØ·?vá>"™ÄQ?¡ÕoÁEÒm?ô413¼?í{¿ÝU9‰?–®š…?ŽŠ'¨2K‰?€›vð?°P°ÀOêE?'@øIAªn?îT°¦µ,?'ÉÙ6Ï?+?Ѽ!?}·
 P‡à?¢ô3µ >F?‹ö(Þuq4FGL J1516.8+3651¿ïíh ÿ@Lñ¾ne8À;"ªLÀ<Ò6/fö@³B§'@
ª]6;ü?Ä˝bQý?·x°ëŶX?ì®Ö™íý@æ]êÁÕM?ÞU?bžÎ¿áåÓ)Þ ¿ÍU*˜ë¿êo¼árKL¿ßœ_Ý
\¥¿×¡CœŒéAGNbll3FGL J1516.7+3648MG2 J151646+3650?ï{3­Oìî?">œéš…·?A±>•ôN?:_uÓÂ@?aYŠ¢?"FìA+b?ïf³h<Ԝ?šë&žs†?MNÏ+õg?b$·–FÓ?'?Ì¹?š0.n<Çg?ît¼rq?:µk²?t2¸•ð-?qŽª''e?¦-çûêÖ¢?ŽÄ.´Œ?i|@…?pK……*Ý?Rgþ )µü?EýÅ(àS8?…È%Üê§Ï?oU¯¼¡ž24FGL J1516.9+1934¿ïK`Ô+:ì@Kð®Bž
BÀ:l3¹jðÀ<]úꉯ@HnÃ>Ú@WC³³÷?½êmœ™ì?oÌ]Ûþ?°¼0Gpó@q[$=÷Ý?ä³½œ®!¿×ö[üÕþû¿ëʝþ-B¿áâ™Ýâí¿âA&»×¿ïõ
8h&ZAGNbll3FGL J1516.9+1926PKS 1514+197?ïë†é®Y?`̙KS)?B·zËÏÐ?=±j3%s ?_˜ï=fô?^È5in?尿>š"M?…­ö0çé??®+
‹?Q:"½†Ä?…S?ò"?"É°á8??îæQú¦ˆ?‡!ˆ¨ü?t†ö	×Çì?l%ð')2?ž;•<ï?…	õ`Ú?ï¶àÓœ›?g!ž1?[ÆÔLa<¬?IópÆËÚ°?}ál™d§?dŒP"5ôT4FGL J1517.0+2639¿îâÙøj›@LÒÂ&€IÀ:¦7åI›UÀ<éᰉ @fâæi«ë@ü¨"1¡?Àæ'w2?˜hͧpÐU?×ւN8ó@«Çæ2)¿çsø`îW¿ÙJzAå}ž¿èxDµ;·¿Øñ±ž6ó¿åTˆM@ûs¿ðAGNbcu3FGL J1517.0+2637SDSS J151702.59+263858.7?ïê§\ý_4?[oÍ~À@7?=%aWjO?38¶8Wùé?a³ñVuÝÁ?XÒ]	éµ?ïŸß²á4?‡[›5¹¾?C6͝ü.1?U÷\E˜yÑ?†Ô¦Ÿçð[?†¨ääÓû?ï9Ÿ
wu?€ï jÐA?k©'õüÚ?YuëJ!Ù[?™ã™ßñv?~üðUï©?ïbï.ï9±?v;k®:¸Y?kÿƃK?TGhrCX(??º)Hf?tn"ãÊz]4FGL J1517.3+6630¿ïA &"+Ò@FZý›¡²À;BŸÿå(
À<ÏèYmZ@̘×ÒºM?ÿJBÉ©+Þ?ÙÚ €a?Úڐڮ6à@u4½vît@^ðù²?âÊ¡¿,ü
?ê{|½ë³m¿ãøÄL0Z¿ç·¡Aƒ­õ¿ïþÁU F¿ìÿ8?®ŠAGNbcu87GB 151628.7+663843?難¥¹r?˜È±ÅÃ?{UáhÛ0¤?{Ü¥VîG?˜5R''?•ëã"ÀÐñ?î|ýQkÃê?¨o¿'_t?|Îïp+_.?–Ç,R^?¤–Lû>Uu?¤'‹"'?ì{u6°ò?Ÿ"à\_ð?¡9Æ '"Ò?Ž|À1¾Å?³‡rúh&'?–ò%
JJí?î'
_Ü?È2¢Úº?‹'Q­¦µZ?ƒTsß<†? úŠòÐTã?ˆvRÞx4FGL J1517.7-2422?Ç%…'‹€@;"ŸDÔEgÀ7o¡vݬïÀ;$óMj@ËBÎܜy@¢U°5½Q?")A9R©h?#59GÊD@À"<jêZ@eŸ±aâ?™—ÿ)‰¿ßGà~ÛRL¿âÛ­p3T¿à¾Q	¿¿äæ
`:Ó;¿à˜ÖšíWAGNbll3FGL J1517.6-2422AP Librae?ïu㦲Z?Œ6(ªr8??|ȳ …d?6Ò¯¡‰Ï?Å˜ñòÁ?‹ëpÀ¨?ïHc&q]€?—¦ógŽN>?bTQ8'0?tfóí0®?"¡ð§­=Ã?–
…[Ì_?îÏâTk¦?˜Ü"|ZIé??ߏ§®œ?€LW–°æÞ?¤èÄOÓ?–cõa£šA?ï"6=ì"7?x'kgåªø?`®çªYœª?US}/˼?†Æ¶šH‹	?w:³ã›1Þ4FGL J1517.7+6525¿Å§¬Ï"à@F²-VÀ9e§Vñ~À<-s?'½@ ®F#û³?û¹9±Êé?«þDZF?°ìȀ6ò@àäJ7\@	ãÔùl"?ïЬU^f¿Ôœˆ Þ¿á,V4¿û-¿Ððú¾øxÍ¿ØlD̸«¿á$¬ó±³AGNbll3FGL J1517.6+65241H 1515+660?ïÍ-"]'£?mÀ¶˜ïªF?DOÿ'IU9?8õ8¾%l?vß=߃Ä?kùhŽ…DÊ?ïZ+×Ûä?Œs)²×Å(?Y¿p¿Ñ?d¬$¯Æü8?"#ãyjb?‰¡<†Â?ï]Œ'%ª?ƒ¤éËž?h¶©24?Z#è?œ}‹,Æ$F?'ÓÊÔ|†?î4Ìiü\ž?‰šÍQÐÒn?Š{zrÓ´?u©5üù?¦yA/?†2y@/'à4FGL J1518.0-2731?éì©OUcñ@8ü*í"1À8×äŠX³öÀ;ÐÞô@ï_íüGd@E^ÿiØ?§¤yá1L˜?'ô;X¬Ñ?ê?Q"W6@©¹qPON¿"Òæí4v¿ÉŸ0²Os¿âVæáËâl¿Üýð;ø ¿ãRÄþ¢1ï¿Ý%[[ÕAGNbll3FGL J1518.0-2732TXS 1515-273?ïëV¿?]\ô`–"J?1ÿdnáA?,êTåV­†?b°vdÄ?[›3¾t(q?ï€]¹ñ¾?|M9ñҕj?>ŠÝbÍ?R
íçÂKz?|×/•0ô*?yØUf•@?ïMgzIá?ˆs5ìOt?kÆ섲…z?e–¹Ôµ×ô?™ýu€ s?†EÇB㯑?ホù²Ô?gó¼Ø?UîyîÅ_Ä?D'±»@?{=Yu=@?eʱ™ '4FGL J1518.4+0750¿Â}OƒmTº@Iãø¶À;¥Š6OGfÀ<϶4ÚÓ @!æ©ÎÅöD?øFc[ïêß?ჲ<'Î{?Ñ[Þ£ˆ?ø@¢òÞ¯M?ÿ8n±d¿ï«¨Å†‡n?Öo'nÚ©.?ïኔC"¿À"¢Êšî¿Æ%
€œ¬¿é5<ø®ÒçAGNbcuNVSS J151826+075219?îôx´æúH?¡DUªí?eGd9¤"?f€Ù-"ù?žÏv™'y? ÑwdOp?ï+n×
?œ'Ñ{®€?ZÌ+T10Ø?sÅÑPˆ*õ?˜áoÙˍ?š.\Ò`?ìٟ¬,? 7û…Æ.{?"'=Ï;?tù"ªþy¢?¶ Úåô8[?žˆ"[¿²?îOû6=Ö?˜5ĝµ§?Q•EÒNßR?VšËqžUG?ªs¢m'h?˜'`?¯R4FGL J1518.6+0614¿ê¥áÚ:@H¥Ç%ÃÞèÀ;NÉ&O"À<¤À²W&@!¶¿•×˜?û·Š*ÍB?È8uý³¦?")ê4;ÆÖ?ÑÁ߇Oj?ýÓ*U"¿ïðrXâð%?ïÿýfG³¿ä·K%˜?ý¿È¾ð€±a¿â›ëþì.½¿¶W¦Úõ¯oAGNrdgTXS 1516+064?ïÒ·+:~?jš0`Xb?3ýö=4­¤?+b+WF²?u»Åvn?i¾¸Òúä(?ï@þ·z@®?'ÁŽÊ҂x?U¦ÚÄÝ-?bò5à!f?–…»o{œc?'²FÄõn ?î1òDÅ¢?Žg:n3?s<žÿX…B?]ÝírÒÒ?ª†Œûȕ,?Œ¢žÉç®?ì,yÂöÜ?C%œŽ©?‰ò» %nU?|¶W^¤?»]ڄDqÝ?$`郘©4FGL J1518.6+4044¿æ[k½#@Lp'À‡D,À:¢"O…yQÀ<¡ã¼Ó[@ *4~6çž?üÕnvÖ 3?½ãpþöÌ?¶Fçeç¢?ú£é~´;@èîݘÌë¿ïýI׺f™?ïúþ§°´¿ÆS&ƒ!ˆ¿ÜèV*¯3¿ßìÑ$o¿Ù<ƒÿS‡¼AGNbllGB6 J1518+4045?ïÑ£Wˆl?i"¢¾Mˆè?R::ß
²¥?Jíà›Ÿ•T?rŸÅfø]9?ec›°À?ï=H³±ÔQ?"4Úˑöo?b× ©ä?oÞJM"Ã?•ûõt¥e?'æ~Yk±?îG=l¦?‹wò¼½?yhf釱r?g_¢ºä"?¨bB¾ø?j?ˆ&#ȹõ?íÞlVz×È?ŽMþê$f?"R+tÀ?€oä£p°?¨'˜}"?‡b}m'+Z4FGL J1520.0-0905?Û¬N֘ö@CwÏÃøõÀ:ÌØU—À<W÷øʁ™@ Ú³€ ?ÿ'º¤ê?ÇX›w•7à?Šû«Uè?Å™bg(@«"ÚJŽÄ¿ïÐ/",z²?>·Ë´¿åÄCá× 
¿ØóY^@'7¿é§Û?×$¿'aAGNbcu1RXS J151959.7-090434?îm¥¡‰ù?¦[ê·ZÜ?pfÈ֟™?f«½Åyjã?­¬L£ŒŒ?¥ÌhþÀó?ïbr¥Öp?Žl÷óN4Ó?RžëLˆ ?]©¸†¬Z
?'‡¼p®?Œƒ1Qä1=?ía68€)¶?˜9çr:?ƒðŽ÷Ӆ?w°žêJÝ÷?²'°*·Ð?•'"nôk?íTܐ8?–ØéùѬ?Žç¯±rüÁ?~Ä¨$êH?³c%Q>¥?•¦·³›<4FGL J1520.4+5546¿åäÎd¯g@Ilë¯#À:‹F¦­~SÀ<ÇúȈšn@29¹µú@'DEª.<?ºªlЍ̇?¥1B#Ÿ?çͬ[==x@²çôE¿ç£¥€š¿Ü	»€Hj¿ä­ÂC±Ü¿àAöD•[F¿æ ß=Ù¿é§E‰w§AGNbll3FGL J1521.1+5543SDSS J152034.98+554256.9?ïT^B±3?­£àAÃù/?h#ž"'÷•?až÷)áØ?'oʳWz¶?­©Ã\å™?ï\)ybTv?'4áÇAí?Txš¤¬ m?e zúB•Ÿ?"3G)j§M?
Í'?î3ȬšÔ?Œ—r¸ÜÎó?€ôZÕçÏ?qT¶ôŒÀ?¨Áø(ÐØÌ?ˆmk"Z?ï.ûèbR?{¿¤fó­:?'ï8ØH~y?j"‰n‰Ï?¨æ‡™VP?uåÅV»óÎ4FGL J1520.5+4209?ïÿýÝQÞ@L÷< À:——sN¬5À<•B›†ä@]"s퍍@*½Bì?ÄûÆnäº?ÄúÒB¬?ùé˜dæ3¦@³ÖwñS?¿·ø·otØ¿è•*™1¿äö3kgW¿éÞá¢Fç¿è_Jþ«í¿ðAGNfsrq3FGL J1520.3+4209B3 1518+423?ïÚÚAk'f?oxÜf$t)?NÄ[ùT"5?O)êÊÖº?mt§–ƒyÒ?l5#Ž±*?ï¤0LwÛ?…D\]¨ø?<Ñ}2³?OoéaÐâ?†
de¸s­?"ürnJ–?îÓþ_M?ˆÜ;žýeç?y˜@±™'D?vמùuuÿ?Ÿ7ïsͱ§?"gX_²ÊU?ïËÿ?¿?bîÑË´µÊ?WrDü'<?D1'â†ò?t¢oná?b´Æ[ 4FGL J1520.8-0348?ïýq—
âÌ@E@j]këáÀ9e¾¶‰"iÀ;ÇҝÇ%Ä@ ®ÏÑ?øÁi÷ë^ˆ?·5ëŸJÞ?Ȑ°|_!#@U¨¸ñ@zkði	.?ïéÐÒj›¿Ò±Ä}óË¿¿ÒƒÒ‡÷°¦¿Å"¨™Þ¿ßÞ¼¹YR'¿äܝàP7PAGNbll3FGL J1520.8-0348NVSS J152048-034850?ì)¼°HÀ?±d¸W",?´tuäxŒc?¬[p,ñ<?¤{I2'åÎ?ž&£Œ²T?åMÂ"Òm?Ε^;ä{?Ë;P'»::?Ì@mjÁŽø?¿N™ö%?³fþ­‡…¯?åÃÚªÛÆ?°Wz"»=J?đåؖ ¯?ªFÐzÀþ?Ç/
¼½ð2?¨Ô(¥¸?ÛU4IGó?´¡ªÉ4?ÁKpՃ?ª†ó<çN
?Ü'Ã>þMK?¸œ'‡ve4FGL J1521.1+0421?å­8TQ³H@GÖbýüÁÀ;<-šlþÀ<'ÐÛOF@¼ú%6ñ?þÝR¦–_?Ó+-€@Ø?Óµàaª@¡B‡N@:à\̉±?ç(-í¤?ïÿáÍì¿ÚÞ;õy"A¿âÄ»á˜
ù¿à¦ºŒ¥¿ïÿ€éŸkkAGNrdgPKS B1518+045?閭;â^>?~Ì1:Vµ?nºk>ÛÚG?p9Ù;ÌXž?}_¬obóQ?vÆCÞ£P?ï;\y÷¾•?–5^UÍÎ?aï
~ɵG?s3ìïð~?–Vq.öå?"jWµs…´?í¸Ž6h~V?"_'ù!§?Ãüý]?€r&%\	?­'"›P?ºÅmÀšj?íÉ­ÈO-¨?–9ÐW¤Ì?ˆ¢å÷Ñ?{×¢EÅ?­<¡÷S§?"IÓrœe°4FGL J1521.8+4338¿è)Ž¡Ãߓ@KÊÒ¡øã¬À:HÚgÀºÀ<P·»*ä@'fuªÑû@DEÅ.î?ÀÐd[õP?³FþÌX´?îÑÕJIÐ@#ö½8ÿ¤1óÿ&øN¿æÌuúX S¿ëÎÊϜ‹¿é^ÑF¯ú¿ïþÔ¡­dR¿ïÿøãúAGNfsrq3FGL J1521.8+4340B3 1520+437?ïù€+Wї?KfÑðôü"?B:"‹ži?Fd¾Ù]OÄ?/¬aø¸2ÿ?6ݶ3K`?ï'ˆ–}Ñ6?—OýSc?e`À¾NÂ?r¨Ö/_Á?˜bÕ|Þ?"¾ÕÄø"±?ïätIäÝ?C2R§›h?r¿úÇ'®?c¶c¬Äº?—þAxšg?fÕ
Øv?ïV!ÙRt?'l?U,?‰òßör&?w»)
A72?Ž÷—"9K<?xôn‹²4FGL J1522.1+3144?ïÙ0B	‡5@L'€uMÀ6¯ÐÈÚÐÀ;,âó¾ý@þH¸Uœj@õ¯¯…")?"}k,fˆ?²LDÀé§@&k9:´0õ@ ^œAk°¿Ð9wн¿â®L·2¿æŒï'zß¿æ»Ráú0ˆ¿éK·ž'QÒ¿ì]Ñó¹AGNfsrq3FGL J1522.1+3144B2 1520+31?ï¶xã˞?…mW®,L?Yñ"vÍ(¡?\¨·#âx?~G)œfæ.?ƒ3×+Ûä|?îckœ*¿(?³³yØQzû?)üς»?'–›2Ú3x?¥~Ç	sˆ"?²"x!ù˜?ïö·±§¶?'B'ÞÉV?ˆ·kJö¬?…U˜ùŠ?'¥sdO³J?‡µ³±î:%?ï¸Üì¤À›?w›éÜ1z?qs •ob?oäp¤'V?ré˜
CX?kdÜs4FGL J1522.6-2730?îœ_΋'™@8fnü7£À8¯®çúÀ;"Ú")=@G'%\@·g2Ë?¦aPÒÖQ0?ÀBLUÄÍ@Ó:aû›@}*x#¨?ïJ?SÒåì¿Ý=E@¿áÆipÜáî¿âeÁ$øÞ¿égM·B÷Ì¿èŠS«x¿.AGNbll3FGL J1522.6-2730PKS 1519-273?ïÃCsÓ?w*1°¥õ?T­˜ã‡¥?UA$î÷ñ?ySøQÍ4R?tËŽ"?ï=}(½?"e7M–?ie—ªfÕ?s/\~0°'?•.H{i?ó#"Ñ£¢?î5èÎ~?š3é¬å?˜ 8­†?'ÝџÇêu? _Õ×GÒ?X _Zš?îOöŸ4‹Ý?ibýVÅ?Š6€ƒÝzû?tc'|?¤rõë¿ã?‰jÿ\ڀ4FGL J1523.2-3941?幞aªiö@,Ï9ó@ÔÜÀ:š
s÷H¡À<&« ,ZÒ@/b™'Y@¥D]'""?҇BlA?یo¤þ|@‡XÅÉ£@ÃNú#"?åg' Ö9]¿×9PC9e§¿á¸n¦¦ÈV¿é*è¬&d¿ïD‹ûbâ?ê,Î?=­‹AGNbcuPMN J1523-3936?Ý$*7Š?È=yâã?Àb3¯>úJ?¸C«5µ?ÚÇÂ	6KQ?ȲV!¤Ù?èïÁwžø™?ú¨CÓ°*?²ãß,+T?µ´ç"¨?ÂÏ
‹n›ô?¼SNY?åð<Ÿë:Î?°m€2,?¾t;?¡ ¢­pZ?ÉùH÷?§ÙöòáŠ?èæ¨qîUÆ?¤ƒ0CoAn?®ÿ?në8?•ÿTؾÛ?Ä¥Ž\‹Úæ?¢70H‰â)4FGL J1523.2+0533¿íEU©Íà@GùÆøÀ;$1âÑÀ<Ô{¦j@ BE‡H´@3c¿Âù?ÅZÒ ãe?q4a†'»‡?¬·øX$Ú@ƒ&ûíKÈ?ﱋÈö~w¿çâ³¾ÞοäӅþÝD¿Ù­_H•p¿èQrÿ&`?ÁûÃ	€AGNbllNVSS J152312+053357?ï?"O!.~?'Ê"v¨½?[]nñ%ëî?[m'̱eU?–W¿,ÇÑ¡?'ý÷Yª—‡?îÎïÆ×)£? ø#i÷ï?b€…ˆdµ?n‡@C[?¡èû:¯"? DKN'?íúNÏ»ãÊ?'›6§Ž(?u+õ½Ú?bmˆžìŸO?­µ¯…žë±?»Š®|?íL¿ëŸ\4?˜'ôIð¿}?£Fªx.v?nV¸bhÃ?³ŸÌ8]›€?˜Vj,¦¬'4FGL J1524.8-5904?Ý1Pá`¿ýªôj ‡ÊÀ90êþ;·À;û¼¤`@ü†x)²V@¿:I§ê?ÀM^7?³Ï1VT'?òá+^R›®@=ÂKIU?ïqéQgÑ ¿äÜ-'€wŠ¿å'/ò?M¿à@RÖfª¿äÇnôªah¿íV ö…-AGNbcu3FGL J1525.2-5905PMN J1524-5903?ãò3J©Ê)?±֫?qÊþ†B	?gûù"ý©?×Ômp¦R¥?ÂwÂPÇ×?Ý~•
"ŒÐ?Æ,xý¤?kIPíÄî?vâ1ee?á%l_åKÓ?Åõü1Ù±&?ãʸDj'Ë?³gÁTZn=?Ÿe«-vqÓ?Šý?ÐmÍ?Öt4ÄSsK?²¡@u¼s?à¶Ýtf'â?¬%ðô©ñ{?—p%
³?|2ùgU'°?ÝnâÄ?« Œ‹èo+4FGL J1526.1-0831¿ï·ôãí$Ü@C$Å~#òNÀ:d'>2j¶À<UW1?=-@ ÞÙꗎ?üèÀ˜áãµ?ÄÔ~\|W¿?ÈaZ8Ô%@2_¦XĽ@(jž"dÿ¿ïí¿‹›ª?ïøÒ¿€#¿ÙHÝòd¿Ø¸ƒ¿'¨¿ê Æê4¼ ¿Ã%I:±ÃAGNbll3FGL J1525.8-0834GALEXASC J152603.17-083146.0?ïVÐYqš?‹9¨p¨N?y$m[U«P?s±¤žk«?¹²ö
?‡Õ_;®Ì?ï6êsvî0?"W²ÞѼç?fS¢!®
?pðr&;¿Œ?–X=Lìw(?¨«|ê-o?íupG*?›N8»íÿ?þ"ôJ?ˆ
›, =´?°þD‰œ…?•k¬¥ü?ìâ롛£5?"n™é¨¨?•…të×9
?~úÄ$ñ*¢?³‡E¸-?'Êw•Gú4FGL J1526.7-1529¿íÂ)Þ!ß@@J#9ÀìÀ:¬ðéÇ´À<f]ú‡;@ |o»Ï¤n?þaÝ4ùÜÐ?ÆV©Zý?¼Ùz°m?öŠ"é9?ýÿrêg¹¿í$

[³?ï鯁7x¿ÐÀ¸âŠ#Z¿á},±8ò¿à	gB…œ¿âçsâOëÑAGNbcu2MASX J15264667-1530269?îþ—gÚþ?"îõ³þ9=?\í)]ðظ?OÄór]0c?ž^@†…'Ú?"'fK…_ä?î­,êEá}?œÁ«F	7'?sÔ®xÒ_?{Ó¼Ï	¸?¢²›˜òÍ×?™<íî7'…?í£¦ÐÄ^?"nÎõÀN;?€™¯p?mûù¡ðÒ¬?°âCñú?'¸8æïï>?éòðŠ?žMÞ#Iœ%? ÷d'àp-?Šÿ«A,¢?ÃùÛ/…Ï?H†²~)4FGL J1527.3+3117?æt¿K¸@Kò`ÐÕÀ: w!ŸŒùÀ;ù"GÁ`@Á¾V<"@;`äFf?Æ? fÒÇ俯ÈԀÜo"?à¡…÷%@÷§f‹Ð-?î†'_8u¿ëIé7'¾¿à§û\,Q¿ì#ã@Òٿłìƒ÷Eò¿ïÿ÷fÔJpAGNfsrqB2 1525+31?ï¼íØ"Ñ«?‰â[Êÿ?SU´Óߟ?PŒ¹d?|³Òb2m?ˆ•‹tlÆ?ïB®ãsðO?•hk>‡ù?UE"GÉ?e՟¬Ä'ã?–UÓphÁ¡?"
®Ê-ã"?íAWÁËH?œtÃ@-6¸?"'{öZLÁ?}Ê^Ù®"™?³e•Ã&\)?™a¾A­û-?îkðô£Ï¸?'é¦Eûâ?`lw¼ËN?]k«ui?¨?éîG7Ù?' ã˜»òå4FGL J1528.2-2905?î8שcñ@6d)¿*åÀ;(9Úí!À<Rӓk@ aOƒöÅ@ž¡%Š?Ç{¹ßµ1Ñ?"'Ë´êz?ÀBE_Z®w@kÈíºX?ïo×ÿ/öh¿ç¥8ž¬þÑ¿Ô܋ò)ô¿ç…L»Q¿Ï¿'ýs2Ó¿çV¯¤ÙšAGNbcu3FGL J1528.1-2904PMN J1528-2858?íÒ÷§ò4?£ûMíupØ?dÇê~ ÷?_Pî×ÌЖ?°Âs_jR?£© Ø"?î'W;6ºO?­@ÀIÌ8–?lÑڗ{<Ð?{µUŠ3/y?«½n£§E?¬qèÖC?ìm*?›¬Cö?˜'óAY?qJñÀ4z±?¶Vد†.|?™4	˜áÉ{?ë‰TœÞWÁ?¢ÿü6a?vÏ¥©	 ?mºT(©ÜÛ?Á$0dX´?¢wý0h4FGL J1528.5-2240?± ¥à |ý@;bÏÃøÀ;7šr­™À<¨©Û0=@ÄøqÁ8o?þ#¨FÇ?Ԁ#[¤Ák?äê<ŸB¥í@SÒz‹·Y?ùQµ)mÇ¿ïÿû˜'2?ïÿjÕþпÂÒ練'8¿êRz᝔P¿ç"Ü0¿ïÿ(3û°AGNbcu3FGL J1528.7-2247NVSS J152834-223522?îzEjGd?¦/<Nèkõ?Ž)a¤Šd~?Ž,æyÎE?§n@8ð†?£s¢–­ù?åþa&~¿?ÆÓà/ƒ ?ƕÖ2£x?Äįµá?Áp¥OÇaŠ?±Ý ¸r×
?èÏÂͳ‹?©:yšI½?¶MQóÝß? š
bçÛÓ?Áše"£Bå?¡«=	"?äAjµÛj®?°¿!ªœ&­?ÃÝ"CîÑx?¬ øAÕ7?Ë2䣃Ð?©áÜ­n4FGL J1529.2+3812?Ù¾¢p5{@K¤÷<ÉÀ;ŽõѨÕÀ<Ò¨Rcz@^{/v:D?ÿ͕I¨À?Ég=üºÑ"?ÁEûø3'ä?ø"¸vÔr³@Ë܌ÞJ¿ïÿæ¦Sf?ïýWÿ›V2¿æ3߀ƒž¿Ú
˜à66¿ÝÒ	L¯Ûû¿ïÿûbâMhAGNbllNVSS J152913+381217?ïßX¬Ç?c]Pbœø?KaÚ¾›p?I†¦s‡+u?iυ6¬\{?_ÁoÂBÕ<?ïnÍ|†'Ï?j£L3ôJ?WìQ0í?dEó
by?µ'ª·I?Œ7,£‡ƒ?î@Õï+ʋ??ŒKË?uÞêFF·?d	 ö ð'?©6ÃÄz€b?Œåät®Ò?î¬"¡:<?†bŒíÜ<?‹9(ý"²?y^Õà	ð`?œâ™
_o?€ÙÐØ&zo4FGL J1529.7+6733¿ï]>ù©¾o@E 'RTaÀ:ø+ìïÀ<Ú]^è@#f½ú!@ÕÓ;{×?Ä:Ôd¬R?³En߆¸Á?îï–ü0g§@•ÀR@Á¿ïâwú ø?ï5Y³Ð|…¿æíUj• ¿ãËЮٝ¿ßÞÖd¦à¿ïÿ€ß֕AGNbcu3FGL J1529.5+6733WN B1529+6741?ïÓ©ž;~?{a¥ézل?I£oÄ'ã_?S5±?‹¼?r÷¸]Em?wH`ý²Ž?ïgh<?‰,"aŸû?BhÒÆsiè?PÍ	˜l?Šÿ˜³ÉÄ=?ˆ-ò-³?îÄ&¥™¤?ˆÍ=ê !D?w"´Wvº?oÂTWGý?£1G
·Žˆ?†g.
/?ï'Ï-TW?pœ
"cPÎ?p©·ò…×?^¼~%!Æ4?'÷XŸheô?kßTâ
Z'4FGL J1530.5-3026?ï¹(Ž@†@5öè)I¥À:"¡°¿P
À<IŠÃ=@ Ûà­T@š¶ÐF?Æì,c‹?º?Á¶Ašÿö?ý,…]T@˜%Ùç½?îåA7Ø´b?áuD C¿ÞA&¦\ö{¿ÛìVÀVë¿äUÜär¿ïÿséèwAGNbcuNVSS J153041-302559?ïl–	Ç]?­(,T0f?v9,ãƒáô?­ÀäcÂS?‰½çf«?aµAÍ$?ï=æN÷xó?•.>sü¬å?hã[#OSÆ?yèò±ÔrÑ?•&'¦÷?'î/±cs¹?íè"ؑ,W?"°û¥Ñ"‰?|åæÛ»¦Ë?p$Q=¥?­á›uŨ?'¯±$êx ?ìI¢riT?™A»÷öÃ?Ÿ¼§Ö…?ˆ¢öcì?µÃïªw|?•ç䘶Ù4FGL J1530.9+5736¿ìL©€0UÍ@HUŸ<pɗÀ:¸Òñ±‰À<̋Ջ¸0@$֐šíW@8‹aÈqô?½+¶g/º?ž.–¸¶ã?âTæA?ýS$Z'hÐ?ï bb ´¿ä	£ý˝M¿Þ†\㔏¿äí·(Ùº¿É$û(Õ·¿ä+4̐fëAGNbll3FGL J1531.0+5737WN B1529+5746?îØÕ<ˆ˜?"q³A[ùw?s®çÙUí3?iÑNÿn2	? 	Õ±¸ä?'MFG-Ex?CÆ=¸? žçVN(2?l'ê%ë–?s›±Ó±"?¤ãí!=k
?Ÿú½Õ"v?헶«-áÖ?",u( ?ìÆ×ÐÓ?tÆRÚH¡n?±±Ë¯÷4?'MÎÌï·Ü?í£b$8Å?"[Ë6´`"?ðÃð7%?€÷ìIª?­ÍÖ¬Àeì?'½£Ž'4FGL J1531.7+4710?à0w'(~F@JpÄÑ¢À;:›!YÀ<çK,N<¤@dªrÚ½ü@ƚƒ¤dÏ?Ä[}i¸*~¿—ïY¥ÉäÌ?ÔsæÂer?ó݋s¼e?ïf[~«Ø¿ìB¾$=w¿»òRÃFfA¿ãŽc¥ÁÆ	¿â?~e`¬é¿ÓS'úð̆AGNbll3FGL J1531.8+4704SDSS J153139.78+470705.9?î²ù"šM¡?žÞû±©à?j/*{¡ M?cš'¡R?£-t¡Ý?ýÐξk?íþß]>lÇ?¨ÿ‡Îl)?{Ê}ªÀ×?LG´?¬˜ºvÁ®?¦ê¢vr?í‰g%'Ø¡?•û»
GtÒ?ƒ>õ—d
?w´ÒÊ׍Á?±Lè#Þîu?"ùE«o¬9?ìßE¶/g?œlp;Ï`?›¾SAí?‹¯J"¤?´!"9´M?˜ö(=4FGL J1532.0+3016¿éqŽ–Â_ó@Kh'£"¯À:ܵxqÀ<\…íë*†@ÐÒ=úâ_?þHH¦4?µ¦â­^Èb?šrFQэ?ä‹Lš† @	'öWµžˆ¿ã¬,ÿ<‹¢¿Õ¢Ô€ËA‡¿à=Œó˜ép¿×®Ué@ Ú¿ãyˆíyë~¿ÝÑLcZî8AGNbll3FGL J1532.0+3018RX J1531.9+3016?ï㸜bÇÐ?^È6Ïm'?6dÅnô)?*Í]íD'?izÊïY©Š?]îG±"?ï›'ÄŒ?Žª¦è¤l?D©gž=K'?VÑL§¦o?‡í…üH‹?PCúö?ïF>Ǫø ?xhX™7Ñ7?c 'n¬êÝ?NŒªÑˆ?"ļËNƒ?vCök—?ï3ŲºŽR?|—q-&?lÃ:DÌQ?S2;ÐM‹ð?•îâ`²a?zà1ùY4FGL J1532.7-1319?¦ñàœ@@Û$Aþ¨À7éï®y$¯À;iTJ0@½†QŒ@‰~Ü~ñx?›D§¤Ê$Q?º(žYÇÇ@{•"d~@€6ŹÞ?Ú¡½àåοÜü""+É2¿âc[Ÿc6¿å
î \+z¿åTw·¿èÖÍÏ2ÙAGNbcu3FGL J1532.7-1319TXS 1530-131?ïÌÕub?r·Ê·ªHŠ?LÁ¼!D&&?Td«­:k4?vc]øœÊü?qô¯5Ú%?ï_Q'¹Uý?""FG‹þ?\!ãÜ«W£?kL˜Qò,?'S±k
ŠÐ?" †ë"¬¬?îÛíÄðµî?"žsd¹À?ŠjŽÍºðU?ˆgì*µ?—LÿûÊ ?ŠÔ)î0~?ïÜî¢c
?b¡6oí4?B#ÐbM¼?7šr—Ï*³?nˆi"s'é?a½<%ò4FGL J1533.2+1855¿âY‰fE¯7@JóFí$À:Y-2h2À<Y´E‹@ ú$…ñF)?ý
fóT?¸CÀ°E¿–¹Æ_ËA²?à'ß@lך?ò,{Þó•ä?î_8	[ÉT¿ä3"âz´¿àù&ÝdtŸ¿Ý…¥;8eL¿Û¢†\ûـ?•_m"îžAGNbll3FGL J1533.2+1852RX J1533.1+1854?ï/ç†c?ŒÌ¶K¯Ù.?g•:Nw¿V?^д¬z×Ð?—uÅd¦Ñ?‹GÚ:Œm?ì^©½«Ì?¶|5¢Ê?œïÿ¶#qÌ?¥Ç%}¦Y?µÎ²%E"?°rQ'D?íG',*ф?–â'?ôË&?…<'ßéXÛ?wýº"??³äB¬HÁ?•"5û*Å_?⁨ÝB	?®³»sf0?³4S[Õx?Ÿ+ÊԈ˜ã?ÖâÉn†?°[»ï…Vù4FGL J1533.2+3416¿ÐI°fÿW@K\
è³³À:4nµÀ@ÍÀ<tݒîY@úŽñt÷Ï?üo[Ømë?¾Q™Ð¡?»Ê³íض?ÿwÑȵ@ǙÚ\,|?ïö&' ®·¿àׇB_ ¿Þåqúfä¿ÆcGãnyÛ¿æ+iÀú)¿Ù=Ÿ¤u–AGNbll3FGL J1533.5+3416RX J1533.3+3416?ïp'STeÑ?€ªyií¤?Y$õ–û+ð?OSAeVƒê?]f<"*?ü
»ÿ+7?ï6ü÷ªË?'Ö'™´ \?d$`–j=•?r
 MDú¤?–›Ô÷ÙWo?k9Ý([?íý1Ò~?'¦Î"Z‡{?{ˆ¢ÅÛ<Â?i7ñn´‰â?¬»Îc&­?ÄêIvó¼?íDu¹å½Ž?Žðîj½²`?–ïôdÖxÀ?|6üW«[?° Uœu\?ŠvoâeR­4FGL J1534.8+3716¿ï|Ç(žâ@K"^þ"vÀ:†®û*®)À<{¦_z¹Û@ -¤f&O @h	¹½%?Á…dXo,ß?tWíÞ²€Û?¨üð-¢P@®?aê«°¿ïþöë"Gù?ïû³ÀsQ¿çác'Å>¿ÚT°ÜVW¦¿ßaÿÏ¿Ü3oce*&AGNbll3FGL J1535.0+3721RGB J1534+372?ïñû…iÇØ?Wò?)(?.ž!uî&?%ëƒÑ3?X50ý²‹i?UÁV	­N?ï©uÅ Œ?…å+qˆ2z?>†Ù‰:âò?Pz'¡Ë?"®"ÂN?"òÒ`»P¹?ïè)o?'yCj…?e–mja·?RÄ\¹¤÷›?®›:?)¿‹€¸?ïWûû"r?wc耭é?nK,	œ
?XÉ#p6?'7ùß×?wWZ(®P4FGL J1534.8+0131?ìq½~ór@Ev¼ÿ À9‰èK®TÀ<½ÅÈ̍@ÆÑÄÙ8k@-ú¡ò-¯?©ã,›Ð'º?¡‡ê<ÒG?ó-ø–2æ@:ñž"S"¿Ì¦bÀi'¿ä­ºþ™"¦¿æRÎÙíFÀ¿åù?¼ ¿æneÆ-¿àËVq_iAGNfsrq3FGL J1534.5+0128PKS 1532+01?ïÝfÈ¡ ?iSÄ-º?5³'sƒ°{?2XEõnÁ?oãîiÈ?h%
üÐÒ?ï¢ÅàH0Ý?'×ÂÄe4Ø?>uµ¢?Tׅá"6?†ZÚ@âÙ?'Ý"Ž…M²?ï/ç0ºó[?"$Û%GŸ?kì¥"™?`Òqsã?–ŸSý@ò?|Õ¥²ã§?ïø+¯…?;ç-ÐoÔ?%þ9¹} ‹?R"/T}?HCÂÓ^'±?8Ƌ7
*"4FGL J1535.0+5320¿ë[W(ÆÙ@I;:h²À:ÙUvT4À<»×¿o8@ ¥D#ñL?ú¿Ãvâµ?Æ»ª¦ds?ºs欜֐?ôŽ¯«SÖA?ú3–b'$¿çª=UËä¿âvþèÓ¿¿ãOb2Ôi¿³à}:"¿ãc܉ٿÏ%ï¨ÄÚ»AGNbll3FGL J1534.4+53231ES 1533+535?ïm͓¿Ù«?…öë	uG»?ISŠIõ½?@D_pò9·?'{±5µ!ò?…'x}ÖU?îŸwѸ$?¡ë@ƒ•È?pöôdý~:?uÑ¥wž•?£é¤WÞû? 'òŸÞ•ž?îa­çà›?&àúÿ[å?unéî!??a¤u€úV¯?­,ã¿"?ŽÝäaFG?ì.Ò¤ãúq?ŠÉY´ó?'K]4ł?6ØUl(C?º6"•û)?›QÅ?5W4FGL J1535.3-3135?ïý­¾¥ÓË@3z'Ä"BhÀ;IØ›ïµÀ<"ü4µê@!¸îžƒ¹?üÁÃiv¼?ÔKí~ÉÈ?ÈIW·Ìàn?÷:Y²ù¼ð@¤Ç¦È+R?ïʺŸ¹¿îegÞ`ú?Ö»&F»¦4¿ÉÌWÇg2>¿æåöŸ..¿"ì Çm3×AGNbcu2MASS J15352963-3133461?ï}H-HE"?˜ªðÏó?D]õ¨¿¶?E=:>á*?hSb£u?˜{DVRö?îîåH·? &'"&/o?cš¨Ç?sÎþÿãNz?ŸÂtõÙÚþ?žÅUŽ9–?íQ(–ûu?œ{Æˉ¥™?w=:Fle?uÜöäNÄC?´áb¨?œ-А…?î:7…?"¦ðª§Iè?dÊhüå?ZB‡¬â›?­š¼é…÷â?"g¸°vW4FGL J1535.4+3919?ì5¥NÂR@Jøââ¸Ç\À:ÎNCYòÀ<½'_Á0·@–À©ÓÎ@çÚaàŨ?Ã#¤õÃ;)?ÅÃ[Ÿc6@S,ÀRk@m‹¿ï‰«zl­¨?ïý_Üßiˆ¿ÝsÃüČ7¿æ¼þùoÿçdÂW(¿Ú¬‡]ðAGNbll3FGL J1535.7+3920RX J1535.4+3922?ïm"²å=õ?‡¨=ª¯?s28vÆ?pÑ=;;Ð-?‹·M|Á?"+Ee9?ïIy近'?"ÄPl&\?dÓ+s=O¢?t'b|}?"6]y¦%õ?¯
v'Î?íȊa'x?"\1۞OÜ?Œ}5«4;>?€»
GÍíQ?¬XÏ y²?•X`ôôb?îÐoyý;Â?ƒxž†•z?"¬\íµº™?€ñM]o?'E³Ò¢Í	?wëс?Í4FGL J1535.8-4730¿í¾iƒë÷#@Ô
ª}íÀ9òż7SSÀ;YË0ëZW@ÙQj€Ò@'þ?5Ÿõ?ʌ×ÿ°ÏÁ?ºŸlÂK¥?ñï_˜@Ê.¿çk(¢¶xÍ¿á­|5Om¿é
߆ã´p¿åd±û.·¿ïývƒ?Ñyé{VwAGNbcuPMN J1535-4730?î#îBçº?©­Ô¯ÙiÁ?`"—ãOEÝ?bc\6°Eª?­ewœ
?©K†¯i	]?ç´Î¦äZ?Ê»ÀùÙåŒ?Œ%S©˜?˜§ÁÈê?ÐëmpîN?ÉÓõ1±¤?è[Y¦U?­~馓lS?Ô_VJPÚ?‰ÈÎ6Ž"Y?ËÜ®žl?«¯·D–?çµ{r†ÚW?°d*é[š5?'Æü*…œ]?pH™¢Èf?Ïý¢s<<Þ?°D0,Rj4FGL J1536.8-3155?ïþm•&:@3…7âÅ]À:˜0òçÉÀ<MãÕ'b@éÿð:»@nÅý0B?Å ¦ÿÝo?»17°pu´?ù»aj~#@ý«Ï§º?æ§,ßÜôã?îŒðÿ1#¿ê¼'ÂåÃ>¿Ëùt`$-¿èû,=WN¿àm­'"ªAGNbllPKS 1533-317?ïVŸ0¡³?P
/ï[?ho76–˜ƒ?dîVìñD?'1e3ö¤?ŽÌ&½Z"m?ï€R®Ä?Xàèî~­?X\ŸVº´?hῬN#?Œêï@d(×?Œ#ï/!¥?î2p·ýf?'qeQfhÎ?{Gìçõ?v¸ûñ•+?©oöã*þ@?GÊõ?îl¾ºÝÅ?ÄŸW)*à?'z´ˆc?ƒÖM]Üä? /Ö÷ßi'?…ÓQâ9΍4FGL J1537.7-7957¿àNu]>
qÀ3rŸb0wÀ9wJ‡ãŽ°À<þ–µº@Cƒbu–@Òâu«}È?±	]Ýçãe?›Z*‡¬Ëê?é´/JWè@'ntҺͿÆzðv g¿âCF;M³è¿å¦ÃMÈ	ï¿Þ5|c¨Ç¿ç»ÿTßUf¿Ùa¶ÔAGNbcu3FGL J1537.8-8000PMN J1537-7958?ïνs›u?l×Õ^Ø´š?C@íϖ@?6s€ZSt?v9(?}ó?kQ+²|ŒÅ?ïāòŒo?Q;
)"?4Pª8¬ô?G<''A?|yüP®øè?€g#Í&Ï?ï/z³{Fg?}ÝöLg¸?g"Ò+š?RÚ3äpøY?—/—Q¿ù?{¸

‡¸ƒ?ïWX®©lv?xÚQ…¥m?lR'É Û?UI	®4µ?'Š¥H9=?vl¿ôz4FGL J1537.9-1344?à˜"LÅi@@EæšÔ,=À;ý>" À<u¡gÄ4x@!ë¨îv?Í?ù6 hUSï?Ïô	Q¸Yx?ÌfÜX$­@WƐr©@ùìðٜi¿ïÿøsCÄ{?ï˜b'p?ïß°Ÿoœp¿¨îi t)¿äŽ¸Ê·H׿…ž:J…AGNbcu1RXS J153757.1-134334?ïˆs1o˜ç?Š‰ÐÛ%?PÊ©\µÅ­?JOÈð€÷?‹ÉÞxƒ
ï?‰±Dø
}Å?ïræb6?"/,=–v?VIL"é?k†ûÔ¿?[YAšj˜?'0ڜ§]?í³ñÎoÃ?–jÃ'?{–Ü™²É‡?iüa"?°§Âì
G?•N8ï>é¤?î-y3N(Ù?—"ZXüù?v:,BŒ?pt+~u§?ªaŕ."?–ƳÓÄÀ4FGL J1539.6+2743?ï·Rñ$×@Jnž²gÇÀ9‡tw¡!MÀ<^c˜UÌ»@c"çQ@…¨¸ñ?®ŒÕ;d™?ŽÐ¸rwÂ?Û@ï~¨|‹@Œ+.,
O¿Ý UàÝ%
¿á±ˆmø+¿åc(>«	¿ã(c@Â	¿èQ¥^ɹó¿Úñ VL<ïAGNfsrq3FGL J1539.5+2746MG2 J153938+2744?ïé–×_§ù?`¦¾Qxé²?/Ö/àÒ?'ÑwLƒð?dkÇ
f'T?_ÁƬtn?ï´y"ú?üñaÏ?=!¬ÞÔO?OEU/_c^?ø«·ÛÊç?sÇkû×?ï82µ,L?~aô¡Y?hÅ*ª¿üH?W*将¦Ä?•á"vý?{é®íà?ïú÷²ù¾9?4–=±=I?$Ö'¦¤?$KþÝm/?>Aý'g"?1j}RˆÒ4FGL J1539.7-1127¿ïˆ3´ØÔ@@ëˆe"¯OÀ:!4–àµÀ<"ý2Æ%ê@ çTWÆ™?ü¨Ö¸ÞÙ??¾KÞ'ñ?¯|©,?ñ¥×Ë-\@œ‡VKJ¿îê´^–ä3?×p6~—4º¿Ó3ƒ$¸:¿Üã'ìý¿Ýt ƒƒ,ƿفí`@1žAGNbll3FGL J1539.8-1128PMN J1539-1128?ïU3£ïŠ?…óIZâ?b¬*òML?WŸYLÔt?"#Îè?ƒÀ&<L(9?ï9Çõ;d?"p»•ÊÐ?bêaŸ€"œ?o"OÔaÌ?–'ZÍh7?'ãåjK?í'õ…Êü‰?˜\ÊÍagÏ?†EüLña>?v˜DÓt¹~?³÷"H	ï?•e3²¦Œ?êg
â­ÚÄ?œ,îlY§€?––ê6þ§?xuɎšØô?ÄPõ˜µ?›žZlWÒ½4FGL J1539.9+4220?á'×]Ÿ@JTøœ^oøÀ:ñ/!U»À<·Ö™Õ(¼@BÉ0`@ÞKÊÙ­†?Ín
å÷R?Ò¹·FRË@Ü$Ts@ž‰XöU?ïú	Iú¿àì5]YøD¿åÑ,½ùf¿ãVq_i¿ì˜FÉ))¿ïÿ韖]ÐAGNbll87GB 153741.6+422719?í.r1ö?«ÕŠgEÏ?"ª6ëýn?ŒÔZ³‹(b?±¥f³t$Ì?©Yeò?íŸîO´ÐT?£Òä–V¼k?‹Îé6Øì?Š'ê\çL?¯
`·-o?¡1Ð&"Ó?êÜþÓÆ?£î>0Ãu¤?ªRoÝ?"FÝfv*?¼çV)æ?ƒïî¡|Ò?ìK˜¥ŠÖ³?—âò]àV?©Ï8ùhÇ?åÈ×¼›é?°»žVõ@~?†Q‰×4FGL J1540.1+8155¿ïŸÇþSO@@{w¯d:À9 *aÓY¯À<ýÎÍX
@  óS
?øÑäcÂG8?±Ò-÷ `?µk½AX@>J`vb]?ÿØ&,dŒò?ïÿµøtñD?¼(ŠbÄñ6¿Ûh1AÁkp¿Ê.ÇΏ¿ÚØ4¿¥F÷¿Ðžñ;º–AGNbll3FGL J1540.1+81551ES 1544+820?î«Tž­ox?¬?'¹›Ñ?{Š»fù +?v–›t¾­ž?¡Ù^¨Iäp?šÄb1Ã?íҕmÍE?ªÑuoàw?v#\]?•IkÂÿk"?ªù ^*–ÿ?¤ƒ¡ƒÅ?ëù:`Ïqý?¡&X¼?•Â žäœ?ˆ;èáÖ?ºÅ"Òöò?žOÕ­"ÞC?çà¬}×põ?ªm'¸äÇ	?©Tx¦ËÌú?"¹^
cOV?Ê(/ÞïHï?«ÅÖÅ!V†4FGL J1540.4+6606?ìXˆùý÷+@E'8\gàÀ;	j²VÀ<'$»¡+^@,B(C–@§£áñø?Åӛˆ‡"Ÿ¿'êŸÛۑ?ÈüCŠOO@¾¦y&¥¿ã3ßá& ÿ¿âHA'O ¿êgÖX€u¿×^ä|káP¿ïÿk»9ýR¿äFù^PBcAGNbcuCRATES J1540+6605?ïÚRR{?jý'ÒÔè¸?]Ü$€D?a¥‰ilß?gys›žÄà?a>\ˆ֒?ïátˇ?ŠÉ),‰9?K^bõÍ?X앚Ÿú?ÑÁvükÂ?‰©É÷ÍÊ?îiAe¶Õ?Œ0	9®}?}ÅǺ?naäÎa.?¥È¦ëÿY¤?ˆâd¸§ÿ?¦äC=?s‹ÀÀ-c?m»NŸkR?avŸí¤?"1¦‡V?pm©µý‡œ4FGL J1540.7+1449?æÄIäƒ*u@Hiˆ;£D=À:EÖL¨O?À<XÑӜʧ@äA:2@57¹«?·`éàêø¿¤$QÛ¦?×e;$C@úV6mzW?ïýÜ9QZf¿æýé¥K¿ä½`t#"¿ÞÉ«…)u¿á¾ÁqN÷µ¿é¨ü¾W7AGNbll3FGL J1540.8+14494C +14.60?æ)®Ã?~C_²í±?]ÌWöؽ?\'Ïéo÷Ÿ?‹Wûv¹7×?{á'AV«0?ï‰úôù²?‡'ü,T]?Jcº@lI?W'?3ë˜`?‹ÙL†Ì­?†OºˆZ^?îl'á¤Ì5?`<""?tr;úþ&t?cMî'>Òu?¦¨šfSwÞ?Š÷í}ØU?¾–w?ƒB.‡iŒ?ƒ'}Ð]ƒ?k!'Bìª?¢_ýÔ¢G?'d*ÛÞ4FGL J1541.7+1413?ÁmK®\ë@H,ü'œýÒÀ:ψ[ƒ´À<€©={‹'@ Œ«hy7?ý|=¸ƒj?Ë6¢Êê?¼»HjýÏÏ?òÆ.jÑ@ÐØ;Y¿â¸J^Èã3?ïôhAÝÅî¿à@ÝݖI¿ÛÜ\AŸ\§¿Ý`½¨"¿ã6«ÃgÉ=AGNbll3FGL J1541.6+1414WISE J154150.09+141437.6?ï3Ș-"?Œäì
X%}?W"&þ¦^|?Q
o[Âý?˜ªçÌ?Œ<Ù£ÛV?ï'2©Sž?Š¾t"^Çý?M2¢ôöE?XFšóúë? +{趦?‰Ï]5¨ñ?î©k$ær?b«Ì"ÌX?t›T¾?_'N`ykl?¬$húG	?Ž£5ՎÊ?î8ŽÇ´?ˆ
—@3R?€m~¨oVË?k€Yƒ€•L?¨dŸÌ÷¯?‡ƒ¦Ÿ-/4FGL J1541.9-2915¿íLnČj@4c†Â&€À:ŸBP©À<3bàŸèh@ h ¢¢V×?ýRÎ8ݗ?¹íY	[ža?¹+œïÑà@¼íƒüyc@°|OG'?ïæ'P¡Ù¿ÖWÀü_©¿Ë߬bôìÑ¿Ôè#ëA­¿âüæÛkÌ¿Ù78+>AGNbcuNVSS J154203-291509?ï$*,CÚ)?Š>hï](?kŠYÇFÜý?aJrGÞ?˜	o>›ßE?ˆ¸0' Q?î9… s~?¥ðŒ^"¬"?†–îMß®
?•e…ᾉ?¨–¬€Ü›?¡H©Ùj?ídÕ@óž?—í–Xq?"Ä̽Œ	°?t	ê?ùJ?²GO¾Fáá?"m`M'Ó?èé:y«œ
?Ÿuã6ó&'?£ÿ¼Á±JR?‡9J±s…?Ç[&èå=D?=+:î|+4FGL J1542.3+1801¿å^ÉÌ3Â@HÜ#|ÜÊqÀ:¦µ{wo£À<\š¨Rc@ù¦&oÖ@ ,ƒɖ?ËhO_8Ê¢?Ïÿâù´âJ?þ‹¾z#²@	Öv·Au@¿ãµ>p~]¿Ùãàd¯,¿èh‰ø;æ¿éç§^~:™¿îRËI?3¿ïÿ2FÄàAGNfsrqOR 167?ï-Í.³"{?"ÄD¼²A?tóc+Ï)?p¯Â§'!?•	^Èüæ?'Š³bW
?î†å
H?§'ÀºuF?tÌøžE@?†7 ,öE?¤øIº?¥öÃUM?횭!SkÖ?—'@Á`Ø?"›ÎBűî?'Å›gâ?¬‡FÉfi´?'yBÔð0?íÃó2«B?"¶¶fÁ|?'FÏäú?x"žpkO|?«ÄmUnØ?'Y¶ìo"ì4FGL J1543.0+6130?Úyi†_Ö@F°üø
Ã7À7‹g‰|$À;LãGb•!@ Ï6K?þdØâ"Äö?•#VØe˜?®vý@Ã@•B½ò%@
˜™êL¿¬"'È¿ÙK'àD£É¿ß´`¥_@¿Þ–ÖZ²Ô¿âÌdȵ2¿åcܺí§AGNbll3FGL J1542.9+6129GB6 J1542+6129?ïÎMÓJà?s݁Nô\B?=o›)?A3ùÝ.ï?wÃ;¤?rêƒc9I?îփÛS$?¤Å!?iÌ 	Yôb?9f3}Â? úøN."?£Yf|°˜?ï­¾)3ß?'íu֏P?'kñFNi?'¡—â
cv?•TO²¶\×?ŠÃómb`?咽ƒ¸>?rÑÀÕ¿R?YjNÆÎì?O&™ŸO|?ƒ6qÕ¹?qÕäFZ|Í4FGL J1543.6+0452?î™HôÄL@E¯àŠï²«À9ð³!*3À<,œ \–Ú@ {ç_u0"?üxœ‰8#?¼W®'¥¹?²á°^­	Ž?ù(¤Ð.@
nòÿ'p*?à8Q_îýú¿è*<´¼4Ï¿áÄö¿w'¿Ô¤Vg®æ¿Ý˅å\»˜¿ßÚD.®AGNagn3FGL J1543.5+0451CGCG 050-083?ïîøt»?T† ¥t
?/&A½•?);CçÜÒ?`U"PÊï?R´Uè79?ï¤mr¼øm?…úrèƒ?Aõ¸ì_Q?Q`IWË5"?…ÅGÁÿî§?"^ÓLê?ï@چ?(Ì[½"´?cô¢´½£?MŽÝ8íZ?šƒ¦Ž?€i8nþ¨î?î#ê›À‹?"T7=zŠ§?p¢R¤¶¨ú?[}"[p`?¤w­"+?ƒ¶/ðL~4FGL J1544.3-0649?îÁ¢(Ö°H@BŸ¸gÀ9%'œüûiÀ;њ#,Tó@ 1ݘL¦?üðI ]?®ÎdÒg–g?«i¾_¡¦-?ÿAVâdå@Nn|4"?ïñâÀÿäý¿Ç=ÈwþiR¿ÙŸ¹Ù«¡¿Û R:µ]š¿àÔ7ŸÔq1¿ÔåÓc¿ÂùAGNbcuNVSS J154419-064913?ïùÌì±ÞÉ?@ÚŒ~?1,&j¡?t0­{?F†'µÀ}??¼F3yˆ?ïƀwª?{|ù7	°?6'=pð?I¤EÊ>ö?{_›W¦?y€:ŬË?ïâ'QL?ƒÿ÷Ñëà?l¶""O­?a"xH?œ,öÓm,d?'*ˆÖÆ:0?ïïUXàÍ?P'Iš‡Fý?ËÚtbœÄ?
œ®¼9t?`BKÓ|S?PuBš*Ñ4FGL J1545.8-2336?ځ¹T0?@8ðgȗÀ:äì-»$.À<a`'÷–¥@"Xײƒö?øpDÖÉ¥Ñ?ў@}·÷?Æþ<"¿j?óYæ/tb@3Z™©‰Ò?Ð0ÿV·È¿í¢FF5nw¿âJßO0j¿¼R—|ˆç›¿×,àÞ§•±¿åï!öÊÍAGNbllNVSS J154546-233929?ë֞q)å?²¬kƋ—Æ?zÍpK±!?p2Wp­†–?¿ª¿Ÿ®ÅÂ?²7Ж¬+î?:]Xí?ªxƒ}¸…?gÙ_œšÚD?t¦*Ïë~w?¦'¶``Ñ?©ÛW>M²?ì¬|9Àg?žõkÕí-7?~Çכ0Àè?ns¾U"Ó?¸¯¢"~ð¼?9ât]̶?é/÷ÜþõK?¨eUÃQã?uÀ°Çh+4?o^ӟ9u3?ʒÈé?¨láUËÿV4FGL J1546.0+0819¿ÝÇ àö$Š@FVV>Ðö'À9¸ÀûÞ2PÀ<)µÆ 
b@×-¹÷ˆ?ü¢HåL"?¶íz—JßÍ?ºÀ‹J÷J$@J˜Yþy@…Éy±ì¿äz-ô/¿âDx4Å«¿ÜYˆœò®¿Ð™:¤É¿ã*T'8T¿ÞÊ^=M'AGNbll3FGL J1546.0+0818RX J1546.0+0819?ïf
 g?c?'/Po"r?b,µó'"d?]uŽ[?øµ4¥ã)?¬ÏeÈÄÒ?îÚßJH>2?š(·)SY?p‡ú§í¹?v¡°ªÅe? AÇ?—GøÿBµ?íÃ
°"õ?"‡|Óåp€?'nJ½(Fê?pzUègó?¯3'P\žý?'$[á>Qv?ëØ8ñt"?•Âelìª?—¢¦ÖpS?€÷šê£®?»VĂôBÔ?"5F?žœ4FGL J1546.1-1003?í"Y`ÛÒ@@Ó£"¯WqÀ:°ÐíÄÀ<1Y²"ý[@ bû0bsh?üqÖ¤?Â&ÂaŽæ7?ÄG0€¦Xš@ú¡ÿ™¨³@\ބ\?ït7àAØ¿Ùñã݊Š2¿ß^¡Ëí)¿Ô¤ô^N¿à½çŒk³­¿ã4…
š¶AGNbllPMN J1546-1003?ïçˆ.¡""?`mÞÉí|ú?Ed¶ò"Æ?C4Äò(2?c£¡Ç·ß?[æA¨Rvh?ﶻšl£¥?ÄbÀÐI€??W©'G]?SìéNÃÀ?V\ŒÁ?€¬ÌLžÃû?îً™ž?¢?ˆgíBvno?p\Ü#½˜?dƒÚìNT5? [ªá¤RÒ?†µEBG?ï#@ìøž?}¡#+BZ9?bký쯶ð?PãÐÙ¶Ì?™Jb£g5v?|¦O¤yª4FGL J1546.5+1816?Åþ"Ënæ@Ho"5ÒIäÀ;¦¸¦¥À<€rmæ@û•b'g@š¸–ž=?ÊçæٓZ?Ä2õö'Â5?ö+—]7@úx3ÃPø?ÂË>Ø,ý¿ÛeEÔö¿ÒZGòÝÙ¿ê\žÊù¿ÖäHŸ+(ù¿ïÿ×ñÃýAGNbll3FGL J1546.6+1812MG1 J154628+1817?ìç[[Ԓ?­Rg~Ò½>?‹îŠð?"¦§ú)X?µIi3Ý]t?©`,¥HŸ?îÞå]vmÎ?™«3´ÄuK?bï®`£ÄÛ?o:‹:+4? â¯BŽæÄ?—Äõ¨Cˆš?íwÀ6MJq?"øm¯«?‰9¬§±D?|¥ÆéX?±ȸŸ‹ñ?'ÕÄ(¨?íÇ?va£ŸK
?|Gû¿<{?oԟX¿ÿT?°Ž(ǾR?ãi^"·4FGL J1547.3-1531?Ã;x,©@=¬€ù£wÀ:ÛºÌð;À<kx(/Éò@!&öÝÂhp?ûTÙý6ø?Ô<Iý·{?Áõ:i³Lô?ò'r…X™õ?ù4Í\i¸U?ä¡ìï'{?çJ{NTø¿ßõ¯¯…")¿äÛî=_Üß?ÅGõâ𥚿åTh!§o›AGNbcuNVSS J154725-153236?ëÒb÷~"?¹ÓÁFµq)?ƒ>ªý1m?¬AtŒHäL?€ËÓR2Û?¶±Eóµ™ã?î>›"¡°B?¨ŽERàÅú?zIÿŠ©?‰£×8ãñ?¨ÔâÌ¥
œ?¥×‡G•A?ì¥wj¨E$?œ=¶)5G"?ˆÌÓg_¢?xøz;v¥?·ÔPêï?š*ºƒ<P?鯄žUâ²?ª
ÆÌà
6?ƒ)Ä?DÄ?ƒÿs&ᓩ?ÈQE"€í?©ö˜Q¨Yž4FGL J1547.3-2802¿Çôµ7ô|Ù@4‹eˆUÀ:FäH•À<?,˜@ ¬Ùuҕ?ý¡ËFºÏt?½#Ë6I¾? ›_æ?æ̆'ø?øC®®(ÇÊ?îÎQfúàÜ¿Û'\:h‡¿áê9Ÿˆñ׿ÜÛÞaÔ¿ßS…
EŽ¿¿½¿¾œ]nAGNbll3FGL J1547.1-28011RXS J154711.8-280222?î¸ëã$Ýò?'y—*ÑJ?lv$ݧ·?a2>J^À_?¢©ßŒ¤FL?Ác°c	£?ìéÇþ«0?´®›Û}H?Œ7ªJün?"2ô'ÜÇ0?µ*ҎÇæó?³¦Üüëæ'?í&äh£(º?—ì †RâS?‡bzo'ðd?wC|ˆAü2?³Ülö\?••Íf…A?æp΍?£ìï¬Í?¦GFÿÜ2?ÊüYÁñ?Ñ5ƒÓd?£–›Ûæ/4FGL J1547.9-6403?í¡³ßɇQÀþã'áïtÀ:†ƒ<`À;Å%ƺd@ò·É°b´@ßå®E"?Î
èuõ¥‰?Òþ¥¢fqÏ@ˆêb		"@ƒ&uµŽÃ?ï·Do›™N¿ã~Qª¿_¿ì&×¥mã2¿ãlja=1º¿ëcՒn,.¿ïþ|AGNbcuPMN J1548-6401?á¸ÁÙ0H?ĉ0ãEZ?ľIÓ³?º¢2¿—‰c?Óë/Wd?Â]ÕKs#P?×I's·À?Êâ<o:0?¹RMZÏG;?¸\–Öbý-?áR'Àì;9?̧œœÈµ¾?Û¡ÿAÁ¢
?±áÒîWZ‹?ÃGºý<?¢é-Ê{jƒ?Úº#¶½_U?°§¤wlÉ?ßtXÐ$|?«Ï;N"1?ÉȶŒêi?«Ä½—6ÓÙ?Ó§™—ifO?ªô´äàÑp4FGL J1548.3+6615?ïòä­$w@E0å£]gºÀ;—¸`.>À<Çç˜*-Ñ@bÿ"	•*@árƒ«Ë?Ãà|-Q¿·H"ø¦?ñrרÈá†@Kžuvy¯¿½;~0\"¿á³—!U<¿ë»G¿1X¾¿œ
F}Ë¿ïÿ¬ž5¿?ïýÝ`˜ÇAGNbcuNVSS J154831+661632?zÝH?½•_â×V?rG!s ÷{?uÆÇLî+Ñ?€ø¢82¡?‰/½EÅ#Ÿ?î¥å€«W?¥Ð¥pKÁ?wÚzú£ï?"hiE	%?¢¦X•ú,¹?žD
PZç?ìÍ•þ—l? .W*Å"%?ŒFhS·u¢?¯?0Ofó?¶žE"Uð?œÖfKJ¯?î^ƒR¢?—ÜV¾>$?‰ï¯GAc?"y‰ÅiŸ?£›ãìú}?"·;J™Z4FGL J1548.3+1456?ëÀ0'¡?ç@G˜–gµñ¿À8ú‡Š£\'À;É>»ýq°@'gh™ò?þ¼#1]p?¨FΤs?ºäÄæ#Šõ@uâXOL@Ý\ª%?ÞÏh=V!Ë¿»N®ä¯l•¿ÞSa;":¿áDÑöØ9¿ã^[`m~¿åÁ‰¢«'AGNbll3FGL J1548.4+1455NVSS J154824+145702?ïÙqCž'È?ò;ñ›?MYÃbñ›Ó?c9Qúüž?o8K‰ÐÌ?zè¿ÕPNÙ?ïM'›_?ü?¾·"\Å¥?ZÅ܊fáü?dZD'@k=?"®®Ëq'i?ŽÑf¥‹¯—?îË
¹Ìö}?'SÐ5"3u?‰SÞ}WÎm?†€çï'ã?™ô¹‡µIu?‡ß…/n–>?ï,=<€ò
?Ím£œ®ï?sô¬mr[º?aSìÞ¿'t?•{-T…'§?}v7–VÄÙ4FGL J1548.8-2250¿ä—´¨@8,Â?«ºÀ9vh<)|À;ÀŒÒá¹Ä@ â×býÑ'?üâh?"z?¬Ï˜ü]* ?£'£Ÿæ?÷«&[´@
6¼ÕˆÞ?ïÿû-2h2¿Ì—Û´q6¿ÑWå.Ãaê¿Ù¥"Ï7á¿Üêö¦""¿Ô΄þ"?AGNbll3FGL J1548.8-2250PMN J1548-2251?ïÏKJãOs?rgd+IAÅ?-E&Á¦‹?#SG¸8îj?wqÈe"9J?r:‡
e")?ïŽâhá&?‰©ßåõ?Q¦øq´±2?`zÇÉ"?Š™×' k?‡t,7˘6?îˆÈ{`ž­?'7ù¥Îx?n ®Ñáq%?h(=yš¸X?¥‰m\×þ%?'|:Õlª?ìeý8¢'ø?›8Ѕ¥`m?†³µ )Ö?mŸJ!
Eë?º?Ä7c
?™øС»î4FGL J1549.0+7846?î¦p8'ä@Ahšþ§±À;çÿ:bËÀ=&(
á'@ ®ëA'v?ÿ³ø`îW?у¤D˜`_?"†`ƃ u?¼|`"Õm@¨ÊÈ»›!?ì¼]\Òi¿å­½Þ€i¿×¾¤kÚ¿Û逢&Ûâ¿ã;ýÂ8T¿Ø;Ä~AGNbcuNVSS J154837+784526?ïŒ'?u'±øH=ê??Öãþpœ6?<:™b7?|¼†9-0?t½zé+½"?ïj2Gn3þ?	šê*?LçZ#/~¯?]óY²}y?'Ò|A ^? ¹Bߥ?íöiÙ¥¡î?"Ë´ó¼?tþMPL?sꌐ+ñõ?­ù˜»¤÷¦?"Ï ïߖ×?ï}Ò&µw?{ϱ"4|?SØ*ÞÆ: ?I9Åzà?Žq¹ÛS?|8ê'¼Æ4FGL J1549.3+6310¿ìZ")=@Eô<³åuÀ;NÊW§†ÂÀ<f<Àz®ó@Àe©}y@>Ü´¡]?»^ò>Kj7¿Â¦jŽ.@ô<¥¢¼X@¯:¥ÃH•¿ÖúüDÿìaðµà!=¿æô'¢TS>¿Ñ£ÌB¹8¿å€|ý ¿Ý¸ƒÕ6oAGNbll3FGL J1549.0+6309WN B1549+6319?ïÁé%½3ï?ƒäRvS?cßÊo|Z?]…Z¥Ú?uˆý<.J?'"âBµ?ï
ªî"[?ßàâ²c?lr CEíL?ˆÍ
âõH?›N%á£?—ÙwƼ;5?îÔôëfx?Šñêæ"?n¾I~§¦?i=ôänv½? Ä̶]n?‰8]ù+?îå\áÙ	?œˆ
H-….?rÍ%|)õ?sGžˆÊó?¬	-2ê?šþêõq4FGL J1549.3+4234?ÞAôuÌú‰@IsŸ©~+À;Z|Tå5À<ì¿\¢˜@awcä«ç?ÿÛãõhÍ?ɘÂçÇ?¿^Ðߚɉ?öH8c܊@\­+qÈÅ¿ï§î'‡Ù?ïýk›Y:¿â™ÝW‰¿ål妸f
¿Ë.×XìÖ-¿ì¨Ä¯ÇÙAGNbcuSDSS J154918.64+423500.6?ïP܂3=T?‹n½Í¯\?fm¾é££±?^¦¸¶|g?"·ÜcàÎ?Š:à
w'?ï{Ó?ÔÁV?Ž/‹SJÒ?Jx¤©Ñ?Wu÷ Wøp?c¯ ä?ŒƒUDž?íã¶Ü/ý?9öó#?Y²¶€Öü?pºo7'?­Ù[æ>5Q?*e]5™?ï;e¯È*¯?€)RœÏ#J?tmž #€?jR·9ù?"'îŸr¡?}"µÔ1"4FGL J1549.4+7409¿àâð7–P@BÜÿ—$tTÀ:¾‹ƒVa6À<±òeÊ@ Œ7Ü:S@EÖٖë?ºw¼úò¥¿®sìôQ?òæY¶T»C?ûn3´ãL¿Ù¢¥œ\AŸ¿åü†™Õ ¿êŠwB+ɇ¿ÒײÄbðæ¿ééâ‡I4ý¿ïþS!æÕAGNbcu3FGL J1550.3+7409WB J1549+7409?ïb߁kWJ?YÅ4"¨–?'ZVø]¥|?€
×ë\¯T?"íȬ̇Û?ˆÀ‹4Ì?î…ðŒ
,?¤; Ê·Å?~ž©ïNt?Žæ¿M—¨R?£Í"m:?ŸF1p¢"Ö?íÐÖήÀ_?'Ä
Qó|?[)Q€ïC?'ÅB÷2ã?«›ÈÀ³¾R?ŽT'AŽÚp?íÉaúŸX_?›§Ö67?£ëë~éáw?—?*8¹ø?žûé®A1V?‡Æ>à^š4FGL J1549.5+0236¿Ãèõ] Ö@DqÔbÃC·À9%[ÚjÀ;ümd‡i@ôÊöˆÞ@òÁmóùb?«ÂÑBÊ¢H?®Ú€Mœ@háa«@¯CWË[¿Õê0_ï(í¿å@ß=è˜Û¿ä¢i÷ë_¿äȖ<"¿ë´	tC¿ïúÓÍ$áAGNfsrq3FGL J1549.4+0237PKS 1546+027?ï¼c¤Pî_?vÆíjâ·R?O80ÜoÊ?B­Òw?}êæÑmBY?uк²å¤A?й­??ÎüÇ3‹4?QIšº9n-?dé	¦²‰o?nXzM'Î?Íû<A	?îÙXâ¦'Ì?Žú¨øYB×?|}}ìTý?tàkÜêâ?µ"0%Ç'?‰¡Rà×é·?ïÙî·Ï~N?_eÍkÍ=O?S»U*1ÿ?Dà™›?l3›i/Ý?Yã"ÕùÊm4FGL J1549.6+1710¿êxšà@Gä\ÈWóÀ;%–'~À<"íٌÏ@½³Wô†@'T·?ÁlIªC
¿¤ú [Ùß?åQ‡F°¾y@— t>Á1¿¶|n¨°¿èÀ*'_–>¿ãÐÂOpV¿å2Át‰À¿ÝËŸŠtc¿¯Öa"iAGNbll3FGL J1549.5+1709MG1 J154930+1708?ï{Ìɪ¥¶?…ËŒîÕ±Z?R5\a•¬?DÁÍS»¡?ŽÆ"	3Ã?…OÖíÍc?ïB"LÁ§;?–ÝdñS#?P)»g‰f ?_!*ƒwý?–¬Ú±R':?•ô8fªJ?îÔÿ':ô?ˆ•­ÑH}?fÏl|Æ?R'$ÈÊ-¾?¡CE¿ï=?‡ÊóºP| ?îàKãKo|?‡Gvó–¶l?Y1áŸ\O9?O**«ªÖ~?¡1²¾N%Í?‡Lcƒ³%K4FGL J1549.8-3044¿ïâ"Ú#2Æ@2' d#–À:§$WÎ/À<h;¤ñ¼p@!"ƒZ=
?ûñLÞÕãÍ?Å/âç¸?¾l͞-ýê?ûŽÍ=5µ@f?˜ò)Ô¿¨è7Œ^H?ï³!ž¶9¿â[ˆAWŽ1¿Ò‰ÞÛÃ	Õ¿ÕJҌ)nŽ¿å-4±B-AGNbcu3FGL J1549.9-3044NVSS J154946-304501?îw'ZÒ×c?ž0ýqˆ?vÛz…'ÔÔ?u•??¥«{"/8?œK¼K®°?îߛï[ ?¡¥o*@¸?iíõ>wá?uÀ3BÎ? gaº"Ý¥? (Óÿh?íL¯äM4?˜½™"p®²?|Ð3 ‰Tà?gŸe¾:Ãþ?³Í}¥Õ?—R¯Þ
ä¦?ê°¯ÃB¿š? /ä.ˆ?–ðœ?">¤M'?ÂkBñc?Ÿ§8€ÄP4FGL J1549.8-0659?ÕÌVÎݍ@A}j@ºˆÀ9=+úYÍÒÀ;ç<³åu:@ÄO(1L~?þ­ÛÛ]‰H?®ªq>lÞa?':Ǭ?ðÄ öð@¦®<éÀN?ï] Å¿Úó)âÙ¿âŸÒ}浬¿ÝT]¥L«)¿ÛÒ_qÕÛ¿Ú@ŽERš'AGNbll3FGL J1549.7-0658NVSS J154952-065907?ïAÚèE"ƒ?ˆÚß
•â ?Zåٜê?P‰SÕí!?–E]"°ì?ˆ……rTü?ïy,t
¦?Œfýí?UGZ¶ò?aã~FÜ?÷¹á'ª?Š!fXçQ?î>øïGoŸ?"ërÚ?xgöû¹?jzˆ"þ?©r,%…8?'{Ä7Í{?íZf¨[gP?'GïšÖ $?þÎKâ€k?t¶CvИÓ?±,ðó¨up?ëé}Ô4FGL J1550.7+7006¿á6ãÝÆ«\@DjËGÀ;@öý»'À<º7ŽÆÞ@<Ÿg™?ò9ìxkL?ÛtiÉÈ5Ž?ïþMþ"7@O×^ FÇ@úL+&Ê?î¶Q•ôÉk¿Ýä©ÍÄC'¿âèj{€)¿ïg/ò?M¿ïŠÿ…†½¿à(6îÎAGNbcu4C +70.18?í‡âŒ=`Ä?µÓîqù
Ç?€ðŠ»ub²?‰ê"Lzp?±¢ÚF¦M‡?´¼ŠÀëR?èÕŸ*?É[ü6d¾?·Ïý¬GÔp?°ۧψ?Àþ­Óm†?¼\:¤©Ïs?èÄ̽Ĕk?§Ð)"—¦Å?´æ/»SÝ?™?×ÖW'Y?ÂäYñe?¢<W²iPF?ç#jŠ?¾zœ4s?™×6°>`?œ¡"5‹ß?Í'Nñ?¾®‰:®4FGL J1550.7+0528¿Á~»7'Ø@EˆÁÛCÀ9œÊ
Õ«™À;ç þ}I@—÷û#Í:@,џšd›?´VÏÅzž?Ç÷Øi8'å@þ‹;26@
èØqÊ?ð¿ß'ü—?Í¿äD£""dS¿ãä'Ë÷º·¿íju>ÆdS¿í4€Û\²ˆAGNfsrq3FGL J1550.5+05264C +05.64?ì÷¸Æ6?°L¤þš£c?©Àº™/ž?¥° ˜–G?¦Ã¹K\ø?¡.FWAqÅ?ì'À	@Wo?·+­o'š!?£®·rVæ?¨l5?!
?´êþZD?°1"çüF?êLÔ‡³?­h02jˆ?¹&>¢È?¥Ä1t*Ÿ?´‡J9E¡?œœAjŒ<è?睆&?"[?¢:U/Þð­?¼•úƱIè?ž–t^'?Ã>ê©
£?›¼ˆ1ªV4FGL J1550.8-0822?ïzâýÄD@@ól½˜|cÀ:ÏR]šæÀ<i‡¿}@!I³	,N"?û¬Ÿ¶Lä?ÒûOyx?¾G¼,@¥¸?ñaI["¤@/—b1ÎY¿ïh4œ¿¾Ç?ã#Mâáâ¿àYÕÿ{u¿â˜TTëꟿÂð@uœå¿áÍâ½ÐAGNbllNVSS J155053-082247?ïƒ@UçÛ?…úe;äµ?:Š`HT?4êÅEØVc?Žcßz[	?…«D⢠Ô?ï©=†–WO?¯!+lÀc?@!þð1?Mï ¼°P?"§®(J<í?€Î¥¨t•‡?íØYˆ?I%?•nØF%«=?qeú6Y–ð?b†ìbǪ™?°&Ô g?""›'_ø?î›ÝE&…z?Œê"2¦?V·>ÆÈB+?Q}EÖVž?¥Œq·afc?:2¼\'÷4FGL J1550.8-1750?ïìp3Í@@;oyB=À:f<OšÀ<#PÐÒëË@üZ.Ì@¹cc}?Áꀘ@Ô?ˆ³xy¶
?Æúw•bÓ4@Šá^<K?ïÿ|ý¬"œ¿æ/N6ĸ+¿åÊWÂ^´Á¿äBÞ6œM¿ïlbäѦ?ã£æ#µèAGNbcuTXS 1548-177?ï(Ò…Å?"ÊŒµ°«ñ?qõâX,M?kA"Ñí?˜]m(ä3ô?"{
Ž¹òî?ï?û+¹?"—QêÕ‰?\»ÀdòJì?iϪ=i¯?–R$"M¤?'ÀZI¿	?íYZÝÿ=?™/ØJ0B–?Žò Ý#>V?€#3éMë?±Xá
kžL?"éJŒa¤?î©a'S£?‡a/!}1¡?}†ðš'IŠ?j¹J듁¢?¡¹NJ¼™?"vý³Hê·4FGL J1552.0+0850?ítJ®`6]@EӜZzÀ:E`Kš2FÀ<b«esø@Æ;óS?ÿƒ>Éijþ?À6+ágC?¿9òj@ƒaŽQ@	ZP1›®r¿êÒ×¾Bph?ïå
`¬B¿Ý™–ÿáL6¿à6çó™À0¿ãš¯ú./¿ê71Åté·AGNbll3FGL J1552.1+0852TXS 1549+089?ïñÓ>[?P7.«Í?Bvž[†¦˜?AZEFcÙ?T‡
¿÷?Ǵþ"`â?ïvÛ¡ë?$üþuA?TFÆ5ãD?aþò`?™£ˆ0ÈÃ?ŒÇ£fHí1?ï?E %Åð?zvg$8ä?h@i]Jt?_ü75äT?•NϤxÍ?wŸ"¼'î?ï3Y;žØß?{mš…wœ?€Ñ+4Öc?iUijxV?'"ïöŠxå?u¼"°¼t4FGL J1553.3+0600¿íص]Ý	@Dù‰7KƨÀ;6Yì yÀ<"¬X¸þº@®qÔX²I?ý7÷¾?ÚWÌOðÙ?êPåË¡T@¹àF&Tþ@ËBhÛ5Æ?ÕÔ:ªJí?ï•÷¹	¡i?â+@š$¿ç²_ä@¿èÒGàê;¿ïú~¯"®AGNbllNVSS J155331+060143?ëÂ:'l^Ó?¶ËÇ¿-û?¬žÛۃǙ?§zëx@6¢?³ž½þÛ%?±`€7aÌ?ë
;kñË?ÀØ¢½hI?­!Ü«sÓ.?µª³¼Ô¨6?¹6J½€
?³QBñú
?ë…a"ùª?¤øa¬-Ò?£0ÔfBÂ,?'JWf?º<‰-J‡? â2Eq5?æü쟧\Ô?µ9ó¡ËÃ~?¹zõ$»?¯ÀÛ,ý§^?ÇNÒøP.è?°˜®wÝ4FGL J1553.5-3118¿ï—Îåù@12—9m	À9Z—ü
¨À;ÃxØXò
@aÖ©?ý'RÛo&ÿ?«M—@+œÄ?µxs'-Â@
žÏc€@S¾	e"i?ïõäRûO—¿Àßȧú"¿ÞÚ/H¥5¿Û˜™ÿÅój¿àÑâœ'¿á`‰ƒœAGNbll3FGL J1553.5-31181RXS J155333.4-311841?ïÎýÿKè?¢ ¦(ëùä?@™¼d0Ž?8­fôrÄ?vq
"¤†e?¢¡K{ö"?ïûè$T?‹ú…¹Ä˜?N ½r£'?]ы'¬
?ŠžúÀÊÊ?‰V¯ñ"?îëí?ü…Ú?†…ŠÔ—em?w,¥|µl?lý:}Êo?œ·.¡Aé®?ƒÿ†Ò¤²A?íé½ÖP"ž?'[*§æƒ4?yAÿžQ?dÈTª/ù?®Cú[ô$?µ2{GT4FGL J1553.6+1257?ÎÇû !@Fš½çXÀ8àPšLGÀ;ÎtqÁä;@ïSpÁ@_æ\ÀË7?¨¿!œž6?¹ÏòF.®@
'âûã:Í@÷['¢Ú`¿Ú"
P»Ú6¿ãÖGj!ÜÊ¿â÷škP°ò¿çèŠÞ?æË¿êOP ,¿ïê=@RUAGNfsrq3FGL J1553.5+1256PKS 1551+130?ï…"¢M¢€?'4îyÊæ?W5ðdÐ
?TöÌ¿òŠ?‹Ð™_ý^¿?'N·æÁ-l?ŸÊ‡ã?Œ ½|ˆ1ç?D¸¦2?ZúӜ,nx?Š	Ý<?‹ø·ã»)ž?îÁ»t2DK?úM«=Á?"cªzÄ?œ9÷ºjÙ?–¼uzgJ?ˆlUOÙ0¸?ïóbø³Ñ?IÐYëOÛ?&tÕF#?«òêá4?WKs÷vÈ?H'«Ç4FGL J1553.6-2422¿Û+
\q½T@6OÙÛ©¢À8²
RÎÙíÀ;Ëãktà @\ê«Úä¾@sÄóºw?§MìGŠ½?¯)PÂvm×@iÝcóÅ_@}ø¸¸îŸ¿»aX"Ì¿àڏbÞòi¿åL'jP¿ãGÉÃ-Ú¿è{ß@í±¿ä@Ï_~AGNfsrq3FGL J1553.3-2421PKS 1550-242?ï³!öÍã?ˆúŽq?Q"‡jÂd?UHKy?õ'_/?‡a¨?f±?ﮉ€1…?qesó·?GVB†?\û´ð98?'ì
v]U?€—Öpæ?ï'aq¾?†æ'k+?r›¹ešJt?e"ß]K ?˜ô0:k5ª?ƒ_ôjØA?ïÌP'A¶ã?dÅç3òß²?RëÅÕ¨5?D
ÛÜ)×?uÅià$¬?bt†;•à²4FGL J1554.4-1215?çÀ'ˆäs@>¨îÙ8À:­ÓÿÆõÀ<S'üžK°@!!šû™hò?ùÑ÷®ø¦?Ñ"ð½m?ۅlÜ!S@pŸ±@NoMjÁë¿ä3ÍêÙþ¿ï®3ïñ•?íé°"G'²¿±ìµàÍ	Þ¿âҊ¡"³¿åv_¢ýÆjAGNbcuGALEXASC J155432.61-121325.7?íÔ¥µÆ?®¼c´ê`?–æ4Œc?>?"̙ुh?±—ʹɁð?¨á³Pf©3?î5}£§q§?¨,Ûúð?‡'"^ùû?˜Ÿ awº|?¦Þ@­Êf×? 5ë½­ôÕ?é^èpê?ªD ,üb?¤2Vu:²"?'ÜãQ@w­?Åy*À;³?¦ƒ™Ò'
?èþˆ¿Wñ?¯›{rMr?">7úô%?‰4–ö?ɞzA·?¯¿¥ée~&4FGL J1554.9+2143¿Ë²Ý|6K/@H
uÍ·À:ºà¨KäÀ<'sϵq@ënºGäñ@Ât֐›?Ê<Kö"±†?ÑqP¥4@‡Š£\û@ó…mèÎ¿éòUóQ›Ô¿Þ¯ë¶pj¿Üž'¨'Y¿å×ï_ô²D¿æITrHù¿ïåXÿöoÞAGNbllTXS 1552+218?ë8ì;çåQ?·N&åop?ƒ Ïì¥
#?~Ô#aƒ˜%?ÁâB–?¶é(rO9?îkDäˆ{ð?£©$@ø?s¨ž
{ ?ut¡á£€¶?¦Öö71Ž?¢¹S.p±?ëü!XY¨ü?¡:z?\z8?¢±½B"_ˆ?')ÛÑQ?¶Æœ!ˆW?—'çf–?í/5^ó?'÷¨l¿B›?×Ĩ/Ó?wŽDÅ*áþ?²PbZürt?òI³,P4FGL J1555.2-4149¿íÔf³U@"
?·¥ôÀ9eR1%;úÀ;rƒ]œ"@š–pÅ:@eÐÄ©Ý?ºB÷ ˆ`·?ÈÏÒ»¤0v@üÿý@öQ'S?ïß¹£ûk¿ãâÑñÏ»•¿ç†‹À)M¿ç|ŸÃF1¿ç:hŠ'¿¿ïüÇ0«™vAGNbcuPMN J1555-4150?&Äöw?¸w~åÔéê?€ª[¾?"¢:îŒ?Ÿ¬EùÑ­U?´mÍ7Ìd=?웳™V?¼ª¬§2v?'L…"úÍ?ëZçLh¾?¸Ø҆Ýñä?»Coƒ"}>?ì|Á<ç§? I³jçÆ?š£!ÞïB?›‡Ù¨¸b?µvù³áò?™›lpzßÝ?épE3ó£¸?¤¾ZÍü?™dhR*[?…}à:÷ÕÂ?Ç^%ì%­?£ncŸC;>4FGL J1555.7+1111¿ïã¶"2Ò2@Eû~|âÀ6{Ãiv¼À:xßN¯|@üØ®,x¯?ø¨–<"?Ž¡öVÖGí?±cXÊÇd@¯b_p¨à@²‡ªƒÌ©?Ù͵à¢Á¿Íù2±-4¿Ö3=ú·k½¿ÐHÏÃL¿ÙQºÀ/Û¿Ù.šG>'óAGNBLL3FGL J1555.7+1111PG 1553+113?ï&iµ´¹?ŸO]Ù7?^IzGß?fö³ú#¶½?™N8gÙT…?že¢ÐØ{+?íþÐÞá"?¹0 Ð?™©¨À͍?©ºE §á?±MŸI@?±fµn1b?èUtK⣐?±©ßL†/?¤ùÑ .'?˜Ì]±´À?Ékºhmæ?°unL¤ˆ?åV{8s̀?¿ð½?›š ›EU5?"·¡'°Òe?ә_…d°?ÀTi"#°4FGL J1557.5-7040¿ïáÈEî:ŸÀ*Odñ`¯À9¤Ãð…8ºÀ</)¹6íÓ@ąrp4ñ@ƪ#T˜ß?³îÅ`ß$?±7Ä<…lf?ýQ‰)ßÍ[@Ž88€¥?ïëÿ,›i}?Öwz?·%¿äV4ŸÄÖß¿Þ»#­Y¿ä5YžVí£¿ænC?ñCAGNbll3FGL J1557.4-7040PKS 1552-705?îc¼XE¯p?›%ώ`j?xW³??p'VvRÇå?¦¹HÚ¡*?˜áú…À=?ìўWà?³h!¦^É?œ«<[ÿ%?¢×‰$ìM?²H@@vA8?®:íYC}>?ëË¿Ô̝£?¡2+n4Ô?'¥šˆçìk?i2/?¼øš·aË?ž™ç¿h'J?çcàÎÅR?©H¯~Á0?¿ïú?¢w¡ÔUЩ?ÂxíC
©? %™Ço
»4FGL J1557.9-0001¿ïƒ2–øvì@BÔÝÖàLÀ:®]Ywj›À<3nUH0ñ@¾x,a‡Ú@ŽÉ¹òÕu?ÑÆláTÄ(?Ê5öHÇ?õ.éÝ~˸@hØë>'¿äùn‡P¿äÏ© ø³…¿áNƒ†1ÝÉ¿ä­¡ŽZ¡6¿î´²ú"¯¿ðAGNfsrqPKS 1555+001?ìö94Èe~?³÷#+Á½?€óžsô?xͦ}¿>î?¶/ԅîUŠ?³§±úID?îõåò@Ó?–é´ÚɶE?d5à[ýŠ?p¢­UN?ž¼'ÁŒeÍ?•1ûëÏÒ?ì¤Pü©$·?ÇÙõÌ
£?›5\¿¥võ?ŠdË/ÂJ?´ êÍ|?–­
š´Ê˜?í=ÉíVXï?—àUŠË‡?uß»ÅÉ?b'\
üd—?´Àr™è?—_ƒäQž4FGL J1557.9-1404¿ª"pmzâ@<Îü›ÇqCÀ;ä܎
ðÀ<¥³7ÐPæ@ë%ŠÔù@U—Ià?Ò)õ1oä"?èQ¤7'M@›ß°Õ @¥õ¢"?ïèçë6D`¿Ï¨ýz>µr¿ÆQˆöÄm¿éprž®"¿íTÝ!®¦q¿ïþÛrýœAGNfsrqPKS 1555-140?â­lÿT?ÂM¾ÛÃÙ?Ï4΢7ƒð?¿ئÁƒ?Æ©Ê>Á?¹åÿOÌó?ÝÈ0«öÇz?ÍÕL#8?Ù4îAl?Ï	â"asö?Âfˏ˜á?³ˆrÞôUN?åÁà'ß"ø?±˜Áøe†?Ľ|mÉ?ªW\'Ö­?ÄãÀ¡BW?¤)
æ|êË?Óre=?°ŒzºA?àa.Ó¥?´É¨/¬¡o?ǖ}ƒ'"ñ?°÷é˜Î5˜4FGL J1558.8+5625?íÓ Y.øï@Fá«\9¼ºÀ99¿×hÀ<J໗@Ÿy•în@iåŸ+©Ò?¬þ¿õ40?­$g_×ùH?ýFÈ •¡½@Úœ&g?ïÌÔÉ'¿äÒ`v¸C¿áÃq~óP¿Ý$O\^¦¿ãwomv% ¿ïÿòß0&¹AGNbll3FGL J1558.9+5625TXS 1557+565?ïôLó{z4?r¹Çh+f?*!±É?"–	neó?T%öäÕuò?r™Þ|yI?ïtAØmÜ?ŠÏ¸#Z£Ä?Tº%\ (?g>§ˆx?,"œŒB(?ˆzwSÉë?ï>²²`غ?€%%s›š?m<0'M~¯?mNwÚø§ö?"'#¡›9(?zCæžy<?ï›®wÃQ?r€Î/ËSú?w6#°˜'è?f1ñÑXd?{H……Ôi?g,»ôߊ¸4FGL J1558.9-6432?áylÿÜÀ!F‹;26À8©1½nÀ;ÒêVJp@²X>…vÍ?ÿA9k[˜­?¤âb¶-¤?—Wºã&'?ñ²žÓ•=ê@פ"G ?ïíH"-§X¿Ù	ÿ}y'‰¿àS™Û¿ÞSCο஗WŸú¿×uq{î8AGNbll3FGL J1558.9-6432PMN J1558-6432?é3*»U?¶NT¥`?t
,u"÷u?n©Ã^."?ʒë°>Ý?µê"iÏ?êÂüséGp?Áušzi¢?lÀžK%#X?}Òuõg>?ā·.Mµ?ÁMRÀgÍ>?êM`àÓ?©PÛåÕí?'ÎiÌÝÂ?'³¨çBèó?Đ¯YÚ4?¦ýF®©?ìÜ·ÍóÙ?œ£ªrÍü1?›ûSÐP!?‡oÃ+ëõ>?²lœS(´?•ÎsÂrà4FGL J1559.1+6736?å""èe7E@DcEŒÒ
úÀ:ö*rDÀ<á‰$@›½Ñb^?ý…‹ûKeY?ŝ^J82v?Â3Eèª;?ú®ç¸5f@M¥ÿX¿Ú(ç	D¿ê¡uÁ"I¬¿ÂA…±ZV¿ä mòKâ¿ÖV>{ë°¿âž8ÀúõAGNbcuNVSS J155856+673646?îÜÁ¨í6?—[¡FÛU?deî3f¤Ù?Z͝WžæB? ø%:Âe?–½š¼%ƒk?ïvö}Ú\?dèdô&?FXÕ ½M?Tøß ¡+?ni›ÀN¦?ŒnHÿ݀?íò©†°Z?'pß1Ü?vDz1º0ä?j͋é8?®ØOí´;?@šô‡Ã$?ïFȍ7Ó¥?zH/¥ˆ´P?b;FÄ/{Ä?Su*ÒhF?"ß…€›á?yÆłåèå4FGL J1559.8-2525¿åô(Ì@4'"àÞÓÀ:^ם
gbÀ<#¤¦©M@éш'›@r=Ÿ¿™?¾húÀP¿ˆ(ÎÓO?ÉÏa<0@|ža)'¿ã_¿"å­¿Åÿ{&<¿çL_ß¹Ž'¿æü¿ÔKK'àD¤¿ìSŸÍ:[AGNbcu3FGL J1559.8-2525NVSS J160005-252439?íõ܈G"?¢ÏÏñÉL?{–ÔÏç;?un#Ý{8Î?­/c­~¦b?¡Óºrw[µ?ïšch…W?"1rž@ÜÖ?B]	EwËk?RáiBxÀ#?ˆAUJR£G?ƒ3ÞՂáÖ?íQÊO$÷ß?˜ôç^
Ú?ˆè‡Ò'¤?ylúḕ=?²TœŒ‡ìŽ?•IcU'`?îwÊ­d&o?†M]BU­?fk|,gøÝ?X2ÿ羆w?§f÷"?†JsÜÛ4FGL J1559.9+2319?âžPøø­@G¹I¾ó(À9ßÛz¹×À<<¤:Œ@7'&«;@^ÁVw?³dŠn-…?q½
«Óò ?¾
~BÑ
õ@
æéI?ê§Tm@?Ý¥h"αS¿åŸÁ}ä1¿ä3aÁ»÷'¿×áËÌòŒz¿íÙ®'O"}AGNbll3FGL J1559.9+231987GB 155744.0+232525?o·l?ò¶?^{(äé{'?Vޗ_s)?ƒŠ>õžuZ?€"ÚØD_´?ï¥jAÏR?…tî<HL?BÃâô3šÜ?SF^ËI™?…y>HñÛ?ƒµÑ××=?îИA‹7?ˆ†ë'û®O?wZôÌÈ??q#ü-ZP? MµD•?…N伞‡?õ'ªñ?q["rßZ?o݌ðú4?atîQ$®(?œ_V¶‡?h¼N#À4FGL J1600.0+8510?ëD7ÒK´+@>Z_¦XĽÀ:š""œÛÀ<Š4 ˜ü¼@tÊUú˜@bÑ6¿?µÞj(ÿS?¢¤Á¦?ë•ÏªÍž"@9"í];¿ÚÜÒČ¿ãÓșae¿áÚ¢þ)q¿ÞacÝu¿áŸÑâ5iÄ¿ìÔUøZQAGNbcu3FGL J1559.7+8512WN B1609.6+8517?ïžÂÉÓ?z]ï¢ÏÍS?_`ºOÂð?Rr	ÆRB?"mA¡ÁEÚ?wþÀ®Ú)¶?ïŠITý'?‰ô‰ì›Y?SžÇˆÞ"ã?a^6¿cý³?‹¹¤Ö˜?‡UðidÏY?î0QC§­?ÚoÒzÛ?€rö¾À|Î?tš)z>\?¨Úm<eû?ŒÁØé×?ï&CÕ¡(–?~3Š×Uùq?Ðq¿"?j¼Æuký@?'OLÂ{#$?x–ëxd"4FGL J1600.3-5811?â:¤"}¾Àœ¾|§ñKÀ9²~'ÖV¹À;³lsÆ¡:@$-"$@©öùÇÛ?¹H'OÐø«?Åz‹vì›@
IˆÅ5ÿ–?ñ˿ɯ?ïýqz–Ÿ?á`·Ð¼E–¿är4ÐÂ$Ó¿á™«ßí;¿çO ~ûˆ¢¿é(ž[ÙAGNbll3FGL J1600.3-5810MRC 1556-580?ÙZÎIåj?Áð4‹…$?ÀS$bÙb?¶ÍˎëZ?Þ{Ÿ"®6?Âp²"<œ?³"nw°Õ?±Uö,‹k-?Ìy[ €d†?Æ
¾ýlÇ?æq&êðÄ?Çg)"2?ál1ý°5¥?¯óÀHÝ,?¶}v[J|?œãÎ$¬PO?ׇ<§Â?¬ó—øx{b?ÀÍ\F÷˜?œ.¹hÊç?Þ~¶L6r?³†Îˆ¨Ò?ٖÓ&¦MÄ?±Q%À ±É4FGL J1602.0-0641¿èð˜‰NGâ@@lÚãæÄÆÀ:ÃÌ­ÃJÀ<J¶¶^Ì@\ÕOÓ'@p̆Uï÷?Ïz4y"P\?Ò_Û\Ý{œ@×z€ÎÇ?ñ"icñÁú?ê¬aBD?íAd®L¯¿á-¹v®³¿âñ.«äö¿é–}_Ò"¢¿ïþ¢NZAGNbcuNVSS J160146-064256?èôÄÉlô?º/ÓNŽ?µgù:GÌ°?°˜çÓO(?Áxð=(IG?´Ò%&ëÕ¥?ãL o3+ø?Ìò"4e_?Ð7}ï?Ëø7/òºz?ŸIqî?µ[•á?èÏ(b`ѧ?©$!§Ü:?³bOË«?™Zßd4!?Ã;-N—5?£Gn—nü?ÒÚôR–ë?­=$ûð¾?Ôí'R—Ì,?¶aâFñÀ€?Ø7yZÒ/è?±µÌ>NÙ4FGL J1602.1+3324¿îÌþy×Ý@HZõÊÀ:ŽFipÜâÀ<¨´ú¬@×	µ5l@k¤"ÈŸA?Á8ø²<(?¾â_&ù?û‹­b¤:@~ôþð
•?ï¥^^Z(k¿¢ÃÂbÀ¿å¯Ö(ôì¿ábòsO'õ¿çÌÀ7"D¿ïõµ>:Î2AGNbcuOS 300?ï ²ú¥°F?'®ó¨÷Â?rÛVrF€?lîÎHød?—2˸pê?eOƦ?î(ò'û? &kUyg?wè£.gŸ9?'Ö·ÿk?¤\qZä?›ôîE/yµ?íĊ&©?"_²^*?‡õÚã
Ø?xrƃ¡?­¹ææߣ‰?ê,ïz¼S?쟧V›@i?"ß²jޏ
?«(
cç"?à*"—d–?ªÝ}2dfi?Š²ìò{v4FGL J1602.2+3051?í?^ÓR«|@H5Þ½çÀ;¹†žëÀ<¼}ÄY@×kÖïí@mç˜ã?ÄÅd"¿H¿¢ã	'¾>r?ý/|&ìþÆ?ïîýy=¿æÊ?d‡¿á5tV2¿ã0‰4LJé¿ÔZe]Që¿ðAGNbllRGB J1602+308?ïڋEÛÈ·?iå¾iø!×?P9Œí§?Kpn!ÌÑ?mWó­hvG?fdvšþ@?ï5˜N0?"B ¸Å?R=ò‡'ªå?Z3TÑåd.?˜8ÍÍÀâ>?'©Øoá?íèO–ëà?'WÇFVÄ?ƒ#ß
€ç?pgÓ;W°Ä?­=™^?ú¼«"í?î̾»ï?†H¦"?~h»2¾Žý?p‹Bðf?žÍùÒ?"Yýá¹,ó4FGL J1602.9-1928?ÙújÞßãš@8C(ÃnÀ:5s"u"*À<([{PÙ6@<MŠ!…@\ޅ[ôó?Òõ»ƒyG?µp$À©¨Û?ò¢êÊ
Ö@ŒrêƒA¿²#½tj5(¿ã6 M}aU¿á4DZ°è¿Ú"UÅYeø¿æTÞÿQš¿éUõÀa¦AGNbcu3FGL J1602.8-1924PMN J1602-1929?ïAêÓIÂd?ŠÅ\=ït}?YWÒÒP?LÄ "ÐBG?–1pš'¤?Š¤áâ%	?ïf¥GÞ´?":$zI>?Hô±Ž?XďU™×Š?‡mö§Ñ?'e¥:)"?î"æl7¢7?²Nwr[?qˆL‰5â?dÐdýŸp?¤«_ ??ŽÃè®T"?îë}U;o?ƒÐ_	°¼I?wïÀ©?Z!YÁ<B,?«#P	óô?ƒgœÛ団4FGL J1603.5-7112¿ïßåä~wÞÀ+đ)ˆ†À:¼ÿc"HÀ<3`:Ó:¥@*Ÿ"ƒªð@û¯S?B5?ËÉB	9å?¹¾'ø?Â8?ñkŠ'•™Z@¯ËE¥Q?ïü	 ?
¿èâÒþ?5 ¿çE^í{Ä¿à–±RF¿êtjÀ¾ ¸¿ïþ°à<4AGNbcuPMN J1605-7112?îœ[›hºË?—®Ù½ üR?wš)RèWÖ?v¯	öUò¨?£GHQ?•ú:ÖÍJ&?íVr-çgS?´Ö(IMU?'ô—~Pž†?'ÆŒL:›?²íÛ ú±ˆ?³Sv$:*Ø?ìÙJ"W¾â?›¼Rlžuá?Œ®U¦LBû?Ñ¥¦ÃÐn?µŸä8x€–?˜
šÚ iò?çy©(d?¤»Uñò?›t.J–Pq?'ºÕN¾µ?έ!ü"d?¤¿Šß†°24FGL J1603.8+1104¿á+t‹JÔî@Eü'œýÒÀ:¤Z7ƒúÌÀ<Kü²m¥ö@ñ< e'@ð?)á{?Áà;êf政U³·µµðB?™¥Zˆ.@‡hÆ=­¿ïž5_³Cå?ï´øÐ`ֿ暉ÿÖ%¿á%ÀN9H÷¿Ù°L£òý¿èò5ÂY¬DAGNbll3FGL J1603.7+1106MG1 J160340+1106?ï±î±±ßE?wÿ?6{F?]oîË[K¡?Y‰Rg`j?¬«t9Š¢?töÖB[€½?ï—iìÃ~'?ˆ".tKô³?Ay]Äâ?Nv–<'@‹?‰-9D
†?‡nnîQJù?í¿š×sK?"jŒÑv&L?€~ólž†?p¤Ü6ð?¯æÒKóS¤?']ý—ÜP?îë‰ÀòB?€¿oŒ3ït?r¹ƒóé$?bgô¿be?àfäÁñv?€&Ñ;Þ4FGL J1603.8+5009¿ïî0wõ"@Gz·ÃPLIÀ: ÌìÀ<§P;¶N@ ,¸¢v³?ûØ	@ñaØ?Âø'6H¼\?Æ1‰Û@ƒÛÂ3?üúWŒ®ÏŒ?鸊à刺Ð8Éà‰B4¿ÅPäÉî¡¿Ûü'œýÒ(¿âK"é\P¿à¿p\‰nAGNbllSDSS J160339.49+500955.5?î¹õ;TŸÂ?–=²×¥?"%ËJ5ÅÔ?{>2qˆ¢M?ž®rðQ$Î?"¸ŽEÕ?ì«}†Ügš?±ž½œÏ"?–wL•œ³n?™–«­}Ð?µ@£µ–O?­7fP‡Î?í'KÙâ!µ?"ÈNlۀØ?‡]ҟ\1?w*t#©?°‰æÝpT?'"y´?è¦àÝz?¡°æéÎp?±ë)4—#À?"§E$aw?ÆÞÊ0ø8?Ÿíýüç4FGL J1603.8-4903?åK,ñr@›†»ÒªÀ7¶Í׎ǮÀ:¹oó­â&@ 4ÞÁÁÖÐ?þ'ü\'?£Ê`0žj?¯Ab\&ؘ@ŸÆ¤"Ÿ_@ô<ö*"(?ï±ÃŸ|Ý¿ãC´VÝ\¿áŸÆ¿l'ú¿ÚÜéåâGˆ¿à…_L–²¿ßt¤9/ÌAGNbll3FGL J1603.9-4903PMN J1603-4904?îˆ3Z*x?ÍéÉ;¹¼?WÏŒi­'?T2­Ç³29?¦ÁSÍú?yÇOfÓ?í˖廊?¶T!`•X?Q"Ë#л?mC1	Ë3?±^¾­žq?¶;¤sQvN?æ"÷!ð<@?°œòç†	?˜pd3ÛÍ?ˆõ=UzÔG?ÑQõÜIÃ?¯ßއC–l?íÿ96?'öF¾ì?'?N¤ð‹HFª?AgÇÁ#Ÿ?¦y}]ßKy?'ÝÍu4FGL J1604.5-4441¿árÓÚ¡æ@­§m˜À8ŸïŽ˜´—À;Žh
/"@_«Jqg@Ez]"?­NÀàãã?µÔšaÂÛ@©ŸâÚU@ÿ]®1S?ïéÌ¢Zˆb¿Ûf&ºÿÅÈ¿æ'f pbê¿âééþ‹á ¿ì,Þ_Ç;¿Ó5nA&:ýAGNbll3FGL J1604.4-4442PMN J1604-4441?í)R½%?ªÚÅwê¦?xLÌgÒzá?x¤Ù-Bÿ?µ2@£–_7?©¾¹ìu?î`,Ìëù?­mƒ‡+?Q*ÊvÓ\Æ?h 2<0Å?©m¶ßz¥t?­e_Ž^ûe?è©X½i´?¬ˆã±eû?ª8mËÏÄ\?˜oÏÌø?Ǽ˜Îh?¨Klk½?í¢r)8
?˜áE÷åˆu?o·É}wÿ£?`|)]lN?±î±Ê«?˜…@ÔÆáô4FGL J1604.6+5714?îŒÁøï{µ@F^4\þޘÀ8¤§.­'uÀ<Õº²@±ÔÎÎÛ@ɐ¢zì? u ŠÜ_?³……žÙt@²¯CO
)@7cI¿×Qaz>¿á¤€-ŒÖ¿æ|fîK¢–¿ä/¥²óˆ¿í•ao0º¿ïÿ "_õAGNfsrq3FGL J1604.6+5714GB6 J1604+5714?ï¨gyÁ+?ž½¯ã-.?pSÛA>?gb~'I]?{ñ,ž?ðÆQá½?î†bRç!­?¬¡iÅ´7i?"Fà`óœØ?žYÅO¤o$?¢ˆ"¹Pýñ?£™å€Ý?î£rØ ‹æ?•åòŽèÛN?‡§f®ÅÊ}?'N"ö¤k?Ÿ½ñ"‹ž?'è–ñú?3)£?y¿}Qçš?'Z«ôµuD?ukûk"&?vŽÃ"Ý?c4úJëE94FGL J1604.7+1734?ïĀü¥éš@FICä/À;(2Æü©3À<£Ø涂Þ@h˜ð§H?ý¨PKqîZ?ÖxŽ·«?ÓÈxª5É@ÖV%¦'¶@üçõG?Z¿ïþ²Þ=°?ïÿ
×ÊVÑ¿Ú%¬!†x¿Ö<« —¿ì¦>Ê.¿ï÷Ÿ¾÷¢AGNbllNVSS J160436+173324?îx]?"ÍJÅÔÉ4?s
M¿.
?n/7@Bf?†]ÕÑß?0qTò-Ç?î³?Nžˆ£? M‰ÍŽ=ˆ?xRʐn‰?€ÙœJÊ.?¡Á±Ä	¤Ã?›zs,a?ë
<Æ%3?¥#¦´Þ	?¨|%Ï÷?"¸¿"J'?»pFÄNm?ŸU+é} É?ìωCã?›«ä‰{?ž¡·ћÕ?'°.¶Ýé?±ÛIVl€÷?•0={˜d®4FGL J1604.9-3414¿ïðÙB7CI@*Û=ŽcÀ;D@\çbÀ<}Rkî@!…çïf?ü-Yvɋ?ØÔ Ö¤¼ã?¼'	AóŠ?ì"D¶v$@½_&V+?ÁóAÁ‰?ïÿ§¬_o¿Þ'{%ì¿Ø~¢u¿Ó$¹½üOq¿æ?,î‡ÞAGNbcu1RXS J160452.5-341407?íÝž¡SŸ?³r&r?Xåÿù
r?W%Gá
?°´Cõ~Ú?³O{h|I^?í›ìw|?½H·Ñ^׀?c]svÏv,?'Ê'íR»¢?²ŒŸi?¼‰œÀ@Ɲ?ìÏr	%?žXžº¥?w"Ïšˆrå?ePS'~;?¸"^ß°?M
ËpÃ%?í
? ÉŽ?›¬êÊ?bžôp´*Á?^¹…dî?·V1Â6?›¸Åá!4FGL J1605.1-1140¿Çûøߋ}@=½ƒƒ­ŸÀ:U%t9ŽÀ<,=CWm¥@ 
ä‡(¨Á?þ'Ï…ä°ï?Ç7y©d<ë?È£}É@-gAW¹$?ýîGSP´ù¿ì!"Þ™¨Þ¿¤öw@(d"¿ÏDYKK¿â:¹ÚÁ6¿ÞCùÿàË\¿ïÿy\ã/æAGNbcuTXS 1602-115?ìíÊ|Ó\?°¹OÖ/Ãò?0@#x²Ä?†¦H>#¾Ñ?´ë§gªNÊ?°ü^—0 ?íÏ7ùX"|?¨LA¨ˆš??Š–B1]¬?b£ˆáÔ?¬fïÞ6°Ý?£ÊÆs.‹ç?ëŠ݁ËÔ?¢§e¹HÙÜ?›%Fä?Š[ړ"Ë'?¼æ,Âlž'?žâာaS?æz_ÅDß?¢Mãz¡ÂÑ?¢\šì/b?‹uGD?п­W•"?¡¸™°¡©4FGL J1605.5+5423¿í@¨¬‡@FƬ![š[À;;¡…÷%À<ém ‹]@ ˆ"Té'T?ú²ÜÌQ$?ËÛTyÿËR?ÇڇËeï?ýšR[íf @ò<˜Œ©F¿ïÿž`¨·D?ïß½4©Tø¿Á0Q"Ñ¿Ó^¢!Ód¿Ý.¿»Â8t¿éÃf½Ë¨AGNbllRBS 1555?ﮪ	¶ÔÝ?v	¾.Ó[?Z_Œ82ì¹?PeƒkÌe_?	ŒDkl?tcby÷‰î?ïg²~òz‹?:!Ÿ'Ü?Uš1\љ?_§ëÂó
ƒ?'°
ïu?‹#ÿ1¢7?î‡7ùÑó?ÑÖz 5ô?{
F£VØ?hlìIË©ª?¬V<—Žuþ?Œ{ÂÖdj?8¿Þ¯?…8‰¶ØW?~q_ÚS?j|Ýñì ?¡øs¶§?ƒk¸|B4FGL J1605.8+7208?åno87 @Bõ¢ß"xîÀ;â©,´"ñÀ=2OŠÎ¢@!LçÂFŒ?öX¡fítã?×
£|ÇPâ?ÕÁ—Å.ô?ö
e´¿@_°
tM/?ïü¬ž"¿Ñì"xK¿î"'r4Ñ?ä𒤲ÒP¿åÖ<b0÷š¿ÁÕ;ƪžÐAGNbcuRX J1605.4+7208?î´ÛŠTdž?­Ý<'°Ú?'DN¾"Ì?©ýòžˆ	m? !3«cq?Ÿ 6'®©?ïj""‹ãÀ?'"G"S»?TWï¡B†°?cÚU?'hto_¾?%-ïI3?쁏ÁêY'? žø©kkð?'øºD~?…ò,à?š×?·u^*bS?õ½8?ïŠîËc?ÏðýW$Í?y`Ð
Ä
?ƒUYÃ?˜¥ºŸŸ"u?‰¼<?T8´4FGL J1606.2+1346?¯¾ÓdìhÉ@Eac^t)žÀ;]™J¿@óÀ<¥äŸQi@"j‰¶¢"?ûG'Æ}¥?Íkè.R#?©ZÞB ?ß³ 9†^@ÌR(–Í¿ïíû@R«t?ïûA
r¿ÛÙÒ#£É?¬öoÞ_Fb¿é2ŸÅ,Å[?нw¤ý%AGNbllMG1 J160619+1345?ï³h{¡Ù?}ɦ—ãƒÈ?J@Lè""ù?EKJ•6?ÜlÕ`9?|¼Ë׺B?ï–Sý8|?‰@´q",…?Dê>sê~]?Sš´ÀÛ¤¨?‰,s97?ˆ(y†Û¦?îèMa?6÷Q£w?zµâ¶òm?qà¦~\*h?«§~~Ó	¿?…o×5?î[½ô"Æ"?L&Å>U¿?wïþw§:%?pÇP².:n?§F ç¾°d?ÊOo°±4FGL J1606.3+5629?æ|vh‰y@Fbb#ᆘÀ;&,ºs.À<Îò`Û+@!"5Á­ßÍ?ûvmÊÞ¶?Æҙ•gÛ±?²;-}'¦?ếBŠ¿@}ã¾V¿ï¯IÏVêÈ?ïìá?J˜«¿à‡Ëp¬:†¿ÝɨÀ~	ñ¿Ã<òϕÔé¿ÞÌDý
,TAGNbll3FGL J1606.1+5630RBS 1558?ï³û
ÅN?'ÑéNÁ?AÓPrä$?7¶²."l?är jÝ?'€Áw'?ï¨æÊÒ?"âó$1ƒ?=×æ‰?LP×[é/?"ݏ®¹šó?ƒH=äžy?îJp»æ.?ŽÈ{³8A?lM‰€Îó?^ ö—¼¨?©"©'L%?O¬S's?ï]C:4?{ýic)I?c0BÈ`œ˜?W$ÐÇÚs?'÷…þŒ¥÷?|)wÅ¡Þ4FGL J1606.5+2717?ä…Ö£æ#¶@Gs¹8›RÀ:"¾³.–À<iÉØü…ø@
ÿ¸\}@¥Áƍ?¿)âýeÇ¿´{ç¾%ü$?ô05½Q.Ç@ÔL\$8¿Ô< A¿¿ç×ä'‹¿æ"[t›¿ã"8^kEH¿ç0=µm5¿å9̪hAGNfsrqB2 1604+27?ï6-™ûm?•cDaó'	?qÅcé¥F‡?næñ¿fÌ?‡O¤®§?"á·4†ð?ïym"©?~NX™[á?QŒÁ´>ò?ej™?Œ¦n7Æ?‹aåñ ¹6?îgª´2²™?Ž±*¦ðœB?y-Ήä‡?fgXPôûŽ?¦eO™Ð?‹'‹!¥?ï~£ó'Z?u›å
ò6?q=I(¶Ì?bclu"Ó?‡ÛrnÚÚ´?qìýܧ§­4FGL J1606.6+1324?Ü>PJù¬@EB¹¡vÝ­À:â°"rÐÀ<OŠë€í@+^a_@'@ô	¢@1H?Ï,—Õõ?Ã,éØvN;?ò œÃÆ@RÐL^'~?í¥"à¿ÙSº|¾§¿æ¹þúFƒ¿âBH§µç¿ê$«°óR¿ïÿI¤ë‡AGNbcuNVSS J160654+131934?ëyjÕB%Ž?°þA¯?—®§ÂÚ?Œøm¸Þ?¾I$«þ?¯f06¥Ù
?îtÚ{ªân?›‡Vì"Ò?t…j«'‰ý?x bàƒˆ?¦!ªï߇í?™VûN• ?ì©ãœ?%µ?œLoãj¶?•]n€4?'™V!>0ˆ?µYœØ«2J?–'¢FÝQ:?ìx(Pp?–C-<‰Û?™4$Ÿ?å|¼µ¾.?¸´q·ötÑ?"{a2ç»ù4FGL J1606.9+5919¿î¯Û5¬pr@EÙßeUÅÀ;X)º
­hÀ=qÞ@‡qÎÏ[?üÔ¾¹
Ó'?Ò+ÖÝò¹ñ?̚Ž…ia?ò‹ºc=¼ú@
^<™8u½?ÙcqT2U¿íR-ÿ틉¿³:è‰@Ü¿ÝÊë€ìúj¿é",<žìÀ¿Î{ÅHIúAGNbll1RXS J160709.7+592115?ï?jÛ¹5?•xÌbøa?eŸàØ¡ì‡?jÇ!bS?•^¨'T›¶?"0qtǦ?ïSPìv˜?"¡Q~ÿú?PÁè/œ?`fÛUü?"‰ÑòªX?'ó›L¡H‹?íŽë+'þ¦?šw¬ô''+?'@ q+Ý?z5Çô~‰œ?±4þŸaåX?™¨Ëkr?ïÖ%Ï?reqê?P°º;Ëó?A!dÙ§?Š¢s/*_e?q'jà3Z4FGL J1607.0+1550¿Ýï"žKÁ0@E³ã*cÇÀ8•Ü¡u0À;͇®µŠ'@{/bÄw@"mH÷Q?¢:ƒ<=¦‡?¼i€0M6@80yþÊ@g~igw³?ïÈtþ¯è¿Þî|µ]D¿äYÝâìпäZÿ**¿¿çp²Osڿ鿞EÐÄ©AGNbll3FGL J1607.0+15514C +15.54?Û¼sõâÃâ?ÄB©'ªb=?³äØt¼?­ÜH—b?ßJ‡Tð?Å/;²?ÊÞ°¦ƒ6×?Ì©n
£1o?åxÙÎ~v/?ÑFŒãœ"?¾{Ð?àØ?º²5êÙ?á'BÝ[ß?±K»,?ÅMEhª?§¾õ¸çúø?Ò4בÎl?°ë_¶s5v?Îòå"éÌ*?®É+îÕÑ?áÞÝ2ˆSI?º_ÆSiê?ɑ¥ ôæ²?¯ú´oÐ,J4FGL J1608.0+4949¿éò"@äC-@G0dÜY2À;d»—cYÀ<ëëºÏ@Œ¨N"5ý@'<?ÓÞ>ɔ^?ڙ‡%"Ï8@8OLnmœ@ék'…?îü'"ø¿©˜ P`¿âôu
œ;¿é5ðè5 ¿ß²¢\¶º¿ïýÿ!]ÉAGNbcu87GB 160630.8+495728?ïl铰d…?œÖâ³þ¥?m²^$s»?s›ÖFÙ]U?YŠÉð?™¦ýGÃ1?îÔ´ƒ"#–?£3úÐßy'?ug=ãhÌÑ?FҒnd>? ÐP­?V¶sùÌ?í="2ø¡F?˜·ýaòý?–¿¿ß#Û?…xÃ1–=k?°cn¥,Ý?"s±U-A?îâ"A¥}²?‡ªF)‹"2?uìø—:¥?lãe'ø?ž49ɪzö?†±'{•–4FGL J1608.0-2038?Úñ(¼Œ¸¶@6'¬dwxÝÀ9㋘O¿À<hXÓ×@…€flÆ}@ž§b¯ø?¶‡a!œÌ™?vàé—çE}?Á>ìdl¼@õ+ÆWgÆ¿åù§4ƒ?¿âEB;å¿âsáxU|¿ÞuÇ,yÜ¿åOv_Ø­¬¿ÕqEiÃAGNbll3FGL J1607.9-2040NVSS J160756-203942?ïŠÉéRA?ƒ#Ã5–÷\?X=ÜÝ.?L4žÆoÙv?ŠK"#´É?'<B?_+?ïª(¨F9µ?ƒòÌÐF²Y?D˜'E"Š?U`õKÃw³?",MÊJ??'½—ôY?î°ÄQøM?ŠDT"Ô?qÍ6Øý?bORJ2?¢Älßܛ?‡gä`ùRf?î¥4Áµ™æ?†tç|šö)?qˆÏáõ˜W?\bȪT??£{™èg®"?…E¿êó+p4FGL J1608.3+4012?ÞÍþâ.ïé@GÊʁ˜ñÔÀ;‡³-¿UìÀ<î™
'¡/@'0ÉKó?û(¥U~Ž?àÒèÛ­e?ᚮÂu°Ü@Q¹eç»f@Yuƒ?ïئõ¢¯¿Ú´ÈÊÍ.¿â›W¿"Ç¿Ú"K©¢¿ïÿûÎBÓ¿ì—æpâÁ+AGNfsrqB2 1606+40?ï#¡'ª•8?'pÑÈê?y ž(+z9?sÍ{Ø»i³?•#³€¢zY?·Ž3Úq?îB±Ë4±?§™£Ñº{?zÀË¿Lo—?Œ®b`bnÿ?¤"»kc&õ?£œYÁ•?ì	Ƥ$ß?¡
ìE
?¥6rC‡3?"c¤é¦?µ+–'½l?—äw^aÄ?îÌgX©b?ŠçÐ²¶?w&^l­A"?uÎò̐®ú? T¾§Ô5Þ?‡,¾­™•4FGL J1608.7+1029¿àDÙl~"—@Dg7âÅ\–À9($}ÊXÀ;æÜ0@úñ£Eë@©æ~Nº?°¦3
9?Ä^DC{Õ¹@Ęވ¶ó@*
díj|¿Ë™à¦ÉWø¿ä«±^²<ÿ¿ç^Á÷†´»¿èÓØYÉ¿ë†Á½¥¿ðAGNfsrq3FGL J1608.6+10294C +10.45?ïŸ
uj¬?€LúT;L®?~ó+O©	i?v­/œ¤Ñ±?q†ûí6?pù1ëÁÌ?ïbH-°?"i.²R'?R¤ELœng?`t Ãíû?'Œ¶@8"?"rÏwŽËÞ?înGS™Óî?•¹"ϔ?Š`·øïœ?€¿C²·'H?¢ƒ\ÿd…?'%ìA÷?ï¶üüïÏ¡?kS¬E}?^!­½ õ?L§®øO#‹?|ùԆÈ?gáӋýó4FGL J1610.3-3958?ïÍqZ`HÀ@!îÐ,ӞÀ8û²êòÀ;hâ·Ý!@O=yÞo@rÓA[#?´&òH‡X?¸'­¼ç&•@| fèl@n'ÏùR?ïÿ1£æúu¿åaRàø}Ö¿çm͘¤§¿ç㺺{'q¿æ%ہp'õ¿ïýYÝl[AGNfsrq3FGL J1610.6-3956PMN J1610-3958?ïÇ€Nõa?tАz=x?6uÄp8?0ó)§Ê+?{î!)ª?s•e–<¬›?캈¥
?¼qcSïÔ?yf·p)|O?ƒ‡b͕­?½èÖ´¸?É?¼+aµh?í6Vå^
?€nôß`º?‹Òpe¼?'K´@½?²ÕwFhn†?™¿o"'.?ë}>×èÖ?›+Ÿ‡'?¡r;Óò?†'A\Êֈ?»‹Ð).ÀA?—¶pÓ>Ç4FGL J1610.6+2414¿ïý4äcAn@F©A(¿<À:ŠŽ›8Ö
À<W[ìà³@ýI¤¹³@@ëGâàí?¹Áµ¢®Á¿¶[¬¤
eï?û=L¬€üë@5ƒo‹©¿áÌ=]º¿ç+{؃¿ë"9`÷ã¿Óe="[¿å£ÚЛŽf¿ÔÎ9´V´BAGNfsrqB2 1608+24?ïLùÖj|u?"½qJFü?p3>þ|Ðq?hsúÊUê?'Sõs=<?'¢þ
æŸÐ?ï_;îæw?'­¸¥ê?Q:‰Èƒ
?^§Óà
Ö[?"õšXæ?ŽS©é&?î/+°Ï7?'øšÍ3Ùr?x†xAc'/?su™pb?©üuêà?'T÷±î/Ù?ï$WÿÂ?ƒ……ä¶Z?qƅ-ïçF?dõ¹¦:Ù?—S´¡Mî?žµ}"j4FGL J1610.7-6648?î}Oó¢À&EÌBcQßÀ80äÅçÖ>À;]C¢ìÿr@m‰'8Ìû?ùÑb§•?£rRØ¿õ?¼fý4ÑC@¯Â¼¨'[@Ëïž]ù…?ïýÆ¿Âx5¿Ë‰ g¿¿ÓPÛ$Sql¿ÒjCÒ ¿ÚÒTჾ¿Þ(ƒÕ,ÃAGNbll3FGL J1610.8-6649PMN J1610-6649?ïyW»BH?cÒdDª?Q+íÍѱ?WGDÍp}?"®ÑÅ3i?Ž‹.1ð?î5ƪʒ?´‰P»®­?}ÔITÿá?šì0Î=¬?¨õjjҖÞ?³:=V¸/?íGÉ]Á¸?¡®!´
žÁ?˜ s¤™`?'ɘ¹M®C?¯…ã0Q—×?›‡K-Mv+?ë<'Z£g©?¦Ú•÷,¦?Œ¬Xò¯û?{Á«æ0?ÁBõGp?¦"øX³m
4FGL J1612.2+2828¿ï
z@FóI{t¥À;j€G¸ü5À<É~#òM@ˆ0,–?þ6§¬Óª?Ó6^á·Àv?Æô$j Ü?òÍ…/?ÿz·^P˜I?çÿMR8¿äwý''i¿ÑE†\{&¿ãþœÞGžz¿Ö`ŒÝž5¿ïÿ®©ÌAGNbcuTXS 1610+285?ï&Úa–y?ïÅ'þ*?oöÍ9íµ?l¨E¶B{	?™\Kz?›eà,?îAa¹?¨Pi3§¡?vR!ʧ¶?\¿n^Òx?¬ÜQ¥«Ý?¦z•\ˆB?ínu­ù_S?•‹!r¦èÊ?…+wáI o?vø:a"æª?±æã"áM?'àL§¼ò?ìp
kn?›ãBW,ž?zJu8Ÿ?p€!E	Í\?½_ß5Q
ú?›€ð(sQá4FGL J1612.4-3100?î³DÁX­õ@-P¯>FŒ¬À9a³õerKÀ;ÐôƒÊû;@µÉ¢ö»?ÿiðÿ±üg?²ÿÂÊí?Ár^—:@¤[^Ëgr@7ºC³3?ï÷T?NÛ¿Û%î;²]¶¿ßö"ºÝa¿ÛüÚ\¿çÄqê('f¿å	BsíãAGNbll3FGL J1612.4-3100NVSS J161219-305937?ïè¤$G?cOOþŽB"?BP—ˆØ–?@ïçBãW¾?bǶ½š?a.\-ÀP?ï™ÈU³8?‰fÄ]a&?O¹‹(°sÐ?bÅÓה€þ?‡Âµ8*²?ˆ2‹r)?îÒ¾Êò'?ˆ€b®/d?X®'p?wbd™B?Ñúý-ƒ?"E߁
4?îðM@û?"{€˜±?qLiïš#»?[ª‹W‰
?ªÃZqW¶?'©S-܍¢4FGL J1612.4-0554?ï¶UôB @?C«CIIÀ:pHD<oóÀ;÷žXE;s@y5ËéÍä@­"'±È?Æ=vƒ? ŒÂ_zRÆ?Õ\cÞл@5H
æš?ïþ_ìÏ¡"¿Ö†—^Uö­¿í´4 ½¿Ó#>ÿP3¿á‡£,ÀRk¿ïÿý{ÁA~AGNbllNVSS J161228-055752?ï«0±j­?…¨ChpæÒ?Q©6£ñ?SWÕ¼t)?ƒ,ÐÖ¥?"Œ¦Ë%47?ï¬X_ˆ|Ž?"\ü›"
!?DLyà"În?c6ëé\èÕ?ƒ¥ ןm?''Í»ªO$?ëS¸W/:?§Sz8¿™«?"¤¢\dP?‡½1-¥`?À<Š_—‹??¥8LRúp´?ï=V¯ù½×?'Ü\YX›¡?gâ|óc9À?Z"Ú`ð?•XÚb[Þ?'Ÿó#Ä÷4FGL J1613.3-1907¿ïÆ	t ¢@6®g¥*ÇTÀ:°Ä±uXrÀ<‰X=@ fÔÜeÇ@™×ºf˜»?Éé'¶Ó;Q?¹hìÓ}k?Æ£ÌùBv@ºØØãÁ?ÒO.¦Üx;¿æ38q`•l¿à㠀þî¿Ùµ
¸A%¿ìÀÊ*Ü?Ó㻹ÿìAGNbcu2MASS J16132720-1908364?æâ/ЉY¦?ÁßwC ?ˆ!?âC?|–©}
`?Ñz–f;Ø?Á€îù<?Â>¦?ž&òÁG;?j!k]l:(?wñcêÑJ?¢³þQþ?šüY™;?ëj"rõ3?£;™g·"]?–¶Øt<za?†róƒ.®ï?¾þ&RI7Î? ×eô»?l?ê0m¡I?£Ÿ‰þÖÚ?{|)ÙM҅?o}Çz}½.?ÆcÖWM?£'¹í"•4FGL J1613.5-4225?È(̊ª
@H)ŒÁDÀ:P#tƒÀ;'I:µL@czðáÿå@€c?jy?Ñͤãú'?·aÓȌv?ìÿMB}þÞ@ˆád3†?¿ïôµ´'S,?ïÿÚáb†¿ìõ¦n"¿Ù±ÙŒÂÇ¿æú"ˆ¸¡¿ÚŸ)ÜvAGNbcu3FGL J1613.4-4222PMN J1613-4225?ÒG1<¢´²?Áöíî(½?‹¶´'wy?‰ž¬–…"?æmŒ¦;Ê?Ây(JLz?çè4?ö?Æaã\¾®?{
Jœ0™?1*>‹Ù?χ:4­ ?ÅËrë?Ùê~3s"¾?±×þª2w_?°É·ÓƊ?"·±†k?á	ǯK½P?±IÚc-YŽ?êç7ÿ®C?¨Œ`¥™M?"ÎvI,?qÊcÉ]Y?Ä{¦8œ´4?¨`­	A»4FGL J1613.6+3411?ÃNJ°þ:-@G0Nø‹—xÀ9*E†òÍèÀ<DÊPñŠ@£KëW@Y䒼/Ç?¦»®—WŸú?Ÿ–k;ã0?óFÌ¢Ûa»@Ñ´ì–¿Îú"€'ÇE¿áýÔ þþ"¿æbE'Ë¿ç~b †ˆE¿à'Tჾ¿ïÿ‡¿ÒhmAGNfsrq3FGL J1613.8+3410OS 319?ïº^8iwÍ?ˆâ~%wª?H0UîL.~?C†šÑýË?ÊÙ
z"?ˆ§÷	`q
?ï€!MÜ?‹Ñ"Jˆ®?Pv"××Ò?`v:'}?ï'Ž	?‰¼ÞkŒï?ï8éíÚ?€ŒŠ9R?iOBGº?\éžûfáü?•ÏÙûȀ?~›Œéùex?ïۊҋý?^$G²'(?\†?x;–?NwxEY¿?f2ɟ7æ»?U'Y™à›4FGL J1614.8-0850¿ám×*b˜ë@=É>¢ÒþÀ;7x"væÀ<_"\h¶£@"җ֜Y?ý+G&/>²?ÆeXŸSl念)f€½¨?𗐪ݎ¼@~I‰¶Í‡¿æœ"¤?¿ìGðI´¿×ôƻ栈¿éùqÁ
{꿳Ce/"§ð?×â•@ÄkTAGNbcu1RXS J161443.4-085130?ìhjZQ«?¿0ùД¤)?PªñpÑ_Z?PØÔ)ìR?¼zg¯bv?¿!ä62¯?íÊÈ]ž,Þ?ºI¶Ì[¸J?uRcUâÁˆ?‰oaÈ!‡?°T–Ý°læ?¹tÀ*'æ?í>£ÔW ?šD€`ÌØh?qÀ&'Ìq?e:ʸ+2?´ú¥ZÙÒU?™Åýô#5Ò?èHVâ×N?»ˆ^1k¾'?\¡çñí?b;BÛOÔ^?Î¥`¦'áé?»©ø¯²ì¹4FGL J1615.6+2130?ïò
Ãl?³@E¸óË>WTÀ9ù9&BÀ<?k@Àºp@˜÷-žsÉ@ëÏkn
?¸aöKKX?¡¶m嶩?áMp€ñ'@\"òB¨¿Ã"ïCDMb¿è8ÁצE¿ëhÎUcä¿ÛÅ0@'/¿êÃJ¢»K¿ïáñ¿Ë]AGNbcuSDSS J161531.09+213011.0?ïïtA,F?haÌaî/?Hý]Èî?CÜÍT"?UÿtxÈ?f¹0U:Ôâ?ï"ü4ó d?"' _N\?Jk2Jénµ?aGNÒî?‰Z?ž‰P?Ž›¶ƒu?ïfÿ<Ž³?…¢´·á˜?pߥC§V?g!†2éÙ?˜»6ÐÝ?Á?ƒ¹øÇØ?ïÓc.ä<?`§!¦¨Âõ?b€'‰ ?S®Y´ø†ó?j?'ö¥?V;"…/4FGL J1615.6+4712?¤g~
}ë3@FÎãK"SÀ:C{À<‡)éÞU‹@å5oùb,@GÇ$_¾?µî@dô÷8?¨f*ßÛ%?òŠFu/W@Ÿ´Ú'³ ?ëw¨¾$¾P¿Ñ´]¸½¿åMI"žˆ¿ßéþ Õ®¿ã&óõ/Âe¿æE£þwiÄAGNfsrq3FGL J1615.8+4712B3 1614+473?ï†]áx?ÐzÅÜlé?^\¥‹†6?NöUÑ"À1?Š¤íºf1d?~kh‰'?ï‰òþ±ž?‰ÚĆێz?Oú"JF-?]ûgR…?‹'ðª†sÌ?‡÷Û>ã
?ï!2nh>Þ?Yxþ¤?l7Xf"×j?^{{Áé?˜RÇ&%‰k?{þÜÆ0øÉ?ïˆæD
?z»º½QÃ$?ˆDýys¶?l5"2=¸¤?ÌdzðD¢?t=2èÆ4FGL J1616.6+4630¿êp¯Nÿ¦@Fœ¢ß"yÀ:ØÐi9~À<-\6@øÓËCµ·@±PÚãæÅ?ÅM-šÂäl?»þÇƨ›j?ñoxäl-@CP¿Ê^ªïj\¿åƒ]b[¿Ä¿éR,†pÈ¿ì2àÈ,T¿ïùÕyC¸¼?ïîê>!βAGNfsrq3FGL J1616.4+4631MG4 J161600+4632?ïßÅ¥"v?møwhò¸?A¡ÏáÙQ?9ç,éì@?l}ÆbC­?lr+]è?îŸi{L4#?­ï›"#->?iôj>´ó?{PßÉÒèq?¤j!§Qn¡?¬5KöbX•?îæŽg>º¥?"UohPÆ`?pÏà8&¾?_ö£ÄÇ3k?žú;
$,?ƒ
Ñþr*?ïD]¹«£O?'OÕ¢ôÀ'?n5šÆ.?`!wdÏ%?"­•q·ó¼?NŽ5AK4FGL J1616.7+3327¿çS
g+Ö@FÖÄ`퀡À;ô/eƒÀ<¯'ÎÉý@g(<	E¤@:#|ÜÊq?ÒÛ<'¦?̍À‡ïø÷?øì#>Éik@vþöj«?ºÂÊ?~Æ¿é"i†¬W¿·™y¹)'¿á`àpÀ¿æëg@ò¹¿ïøUFƒrAGNbllNVSS J161633+333043?ªÇþL?› d³ô¢?s¨Ó|üX?j'^ð(tk?£¢šãàC?šAl
¬Š?aPÞs?¡©ãÀ´si?fýïØ
?q…¡%HYÚ?£—ù«8? ¬Ÿ`O¹ƒ?íµô¾Ã?"P?OeÐY?"`6M?v^É¥§?¯ˆ²'2 "?'¿n8J?íòÚ,»c'?À­xð?z\$5Jw?e}‡¤:g?­Ñ¯Ã?ŒJ«†<x4FGL J1616.7+4107¿åగ7½@Fúù3]$žÀ;îgQGñÀ<ÝÌúïõÇ@p@'Òë@Rºà;>š?ÇFBšvØ?ÆðÀU?üª«õ¼°@I+®Ús~¿æÿb`ÈAο³ï(nß¿æ''àðp@¿ãk¥Õçþ¿êžJ''¿ïÿý¡UûŠAGNbll3FGL J1616.8+4111B3 1615+412?îu2¾?—Ï}2z[Ã?‹f}dÓûÇ?""ŠžÇ̚?žžB,?"i-'©M'?î˜8=Go%? D)³ø ?q$ÀÄ( Î?u«ÆŒÎ¯?¤Wäù°?ž£wàd0½?íG
ªi?™ÔJÓA?•N­B?"\/ýŒyL?±ú7Fœ.?"÷²ï=i­?í£ýåo_&?AgB?œ˜ñŽ?'Ÿü'
z?§t°†Ed?šÙ‰3¤4FGL J1617.2-2535?د€CºÈq@1£Ï_ND1À:a-ñªÓÀ;Ñ}‹Q@ïՃ)Á@™ð^¢LÇ?Ð;¹eç»?×ÑË9NÖ'@¢þ'Q~x@ü¹"`ʛ?î´º𠏿ÑW³°œž¿áÌþ ÚU¡¿éÒI
{¿ël‡þ¼'¿ïÿþÐñAGNbcu3FGL J1617.3-2519PMN J1617-2537?ߢ¾¼Á?ï?Âjuéÿç{?ÎuAN~N/?¿úïö­ž?Ñ" ›ÿ˜ú?Á'å/F?äg­ðö?Å,©?ÆûŽK'A-?ÃQ¡Íš'¼?Çhü«¾û?»5À&´?ß^ㅇ³6?²g!Nàû(?È/*K]?¥Þ­Ðáü?ԉ"å7§?®hçE"HÚ?×&Ĭ?¥NP银×?ÄÛ²XֆX?¥æ#wh\?Þz·ÐÍ?«>¬UgÍD4FGL J1617.3-1513?ääÈԒ
@8†Šar
À;Dèg]À<¤Ú/­m@ t‡t~8?ûÞþ'¸«®?ÒÃöúȳŽ?ã$ì^¥«@
ü«>݋a@b§¿÷ý?îA$øÝÌÏ¿åwÿ ´•ô¿Ã"žWïU8¿ÑM²¥Ú¼¿ä·Z¿êU¿ïÿl\I¬òAGNbcuNVSS J161713-151058?ì÷ÖoËb?±Îì‰þS1?´œ€B$Qœ?¬yîb?¤ç'º¦µ? ÕjíR5S?ãÅ«!Ö?ËµAÌ`=?Ψ"Ar2?Ê,¹ü0?ÂA1^ms?³+á~†#b?èév}ƒÐ?®'ú6"ÿ?¸cÝË)?¥z<õՐ?À( +<?£pxø$»?Ý%¶6â?¯â#‡Z?É ¦î¤ç?°aSË×MN?ÖS†ÒÈ©?°¬Ísbn4FGL J1617.3-5849?￱'ÍÀ¶R7yÀ9>Ì?ß À;"ˆ9@"שÇÁ@ŸÜ>Y×ã?µM16-äj?Î;y}ÅR°@Èa-A'@NÔ¤\–?ïÿ¼®q—ó¿ãJ;ÝüŸù¿æ^:é
5¿æ2qôÆ¿í"t¡'Œ_¿ïýÍ ²<©AGNfsrq3FGL J1617.4-5846MRC 1613-586?ï+'o©5?–RtWí?—& yív?‡¨%"‰š?'Â>º bŒ?ŒMð4Ú­?ëQNÞ׆M?¸'¾?p{X¡œO?|Ðy­jMî?Â6鿕Š?ÁùSÓ+ò­?èÆ~Àå+?°"Q÷ʲk?¹Ö®R#U?£›K8ë®ü?¿õ[¦¸"?¥tpƒkô?ëÄaõµÛî? K9:d¬Ë?Ÿ‡ÿá쉝?Šž7
"?¹úðYÕþ,?œÊr­¸4FGL J1617.9-7718?ç²î–2˜À2ÞM;òõVÀ8tvÔr³|À;²/,=u¬@‹Rùw$Ð@ƒ'?	*K?¡.—3M_?¼¸ÈúÃ@À‡Þ†2µ@©Ö¨˜»¿ÖýCãÅÝ¿ä…dXo,ß¿è™Ì$0`ñ¿èH*;<ìð¿èS½í5øà¿ïþRúÉAGNfsrq3FGL J1617.7-7717PKS 1610-77?ïïàä'ç?R78c—Ô?GuàÎý»?BûBþ5?TƒF™ü²Ò?K5´ÔÙBÃ?ïºE4³€?€u8•íB?@™Ój]v¸?X?Wýdƒ?€eœ˜H³?€6!Õ?ï3‡^©#‡?‡GEºÖ,,?v/Îí

?sPý/µ¶?" o˜Kë?ƒënLøÙ[?ïÏFȄ Ñ?eêí"uaÝ?Y+4P»e?L{Ž¾Ûû?rΩ€¾¦?bâñh'i4FGL J1618.0+5139¿¿ú3ÉlVQ@F8AVâeÀ:Žf$ø
À<ž0´Ó±Ã@Ua÷ÁÃ@†6Œs?˦>m£ò?Ìd6÷—&?ýñ¹KÈË@µ"Üž¿áÊ~ŸBP¿âÐ{÷È¿ç=xÁ‡Ê9¿í8Æ_ö4пåF/ßÁœ¿ïöØmAGNfsrq3FGL J1617.8+5137TXS 1616+517?`ïE?¢çh"±¯-?côY²|Π?ˆF5³û½E?Š¢'W…Ð? ‰\Ùè?Õ?'RõQ¦Ï?Ecðÿõ?_ß¶m?ŠÛèÛ®•?'µ"¾Ú4?î/ÅäæH?'ÏÕù…"¥?ˆöp4£{?mµÃ§ì?¦Æ+U¤r™?Œ—´¼Æ?ïç£!éA?TK,Œ,?9f{ýM?(ßޝ‡Å?e9±GŠÞî?S	\w;‡4FGL J1618.8+0620?á¡ãü$@BQAAé¯\À;5¢é¤sèÀ<šè¯bk@*s6›f?ý™yƒyœ¤?×3Úé%?Ô¹‹|uqq?ûŠ'5Îï@ëyÙ	ññ?ï¶`^åh¥¿ï)BUæ?í1Ý'ãƒ¿àtž7ŽÇ¿è÷ôÎs•ú¿â.ó2'#"AGNbllRX J1618.4+0623?íBÍòÚ?³cq
6Õ?" º–¨?x-?A)?´ÓUŔ(?²y®žnÂÅ?îéþz&þž?ž)O¯³°?kÁÊÍwØg?y?{ÊK?ŸG÷aq1	?šÆC–
?ì>EàéÊ·? 5N\£­Å?"Öü¿G È?ƒÊ.á«o?¸ØÈßâ?œàÏÿ­ä¨?íå…&´d?™öµ†—ßß?r£^(h? ?r
µƒl?¯SB˜‡±Ý?˜óeÎÇ)4FGL J1619.0+7536¿ä{¹šý@A¨ôàM/À:˜NHboaÀ<Ç>óZÖ@7*Èü@:dÜY?ÁØÍ÷o7Æ?ÛŽd9îí?ÝGåœÒ^1@D qúï¿Ò3 ~O¼+¿æÌè`§	Å¿âߟb[j¿Úa(	3…¿ÕÙôÌ.A¿ïÿÿ&¦³AGNbcu3FGL J1619.1+75386C B162034.5+754454?ï§äAñ»2?zl™q#¢?bSÕüW;V?\¼T¨ÜŸÞ?qú{dÅ?vŒ"B^?ï'òëiÝÛ?…«Î[_3?DøŠ"BÌ?S÷qAÇÑ?ŠµœßU?"¿±œ@ƒ*?î,š.8E¦?Œ&^)‰Øï?xk%l$o?j6Š¸"ä
?ª(øjŽ!
?‰aQ~¯,)?ï(¥÷͜?yÎf®["é?qR|ŠOüä?[ón·:ü?–©ÌrMK?xë3€Å'4FGL J1619.0-8346?í¼Ö ]æÀ71qâ›k+À:õ6¥®zÒÀ<.Ï d$@¸½Mþ»‡@ú?¤Z½¼?ÉõMõVXÒ?¶s€wµ?éؽf'|F@,9í±?ã£Æ
•ê¸¿Ú•yyh¢¿à»²]µ½½¿èA•\¿æ;Þ§j¾¿Ì9\-AGNbllPKS 1608-83?îÍcÄ#–ç?"Á*'vÎ?bü«±2§?Wkˆ2]Q?¡ùù«~~?'ˆk×9ãr?îô3
"'?—`^I@Y?`jÖ÷cÑ|?hóqðv\?ŸlCá3¿?–e¢F@·Ý?í™ÏÀž9§?'­‡_9ÇÖ?‡Ø÷әú?všpóȧ_?°N&Ü¿'?ŽÖ¥ŽÛ?íÔS¼£u?ªmY?}³>Æ]5ª?iö‡…þút?¯'ëj!ú?ŒÖ+™ø»‹4FGL J1619.6+5536¿í'PÆÛµã@E¡Þ?»×²À:†—¨'ÑÖÀ<³¯' Wú@5ÈRi¯F@õÀ[¥BD?Á7;ÀöTÛ?À¹‹§h6?ûIKRä©b?ûÜP§¿¶abEšh÷¿ä‰»j¤¹ˆ¿åê™ÑͽŽ¿æ]¤öÄíÛ¿éÜ5 uÖÇ¿ïý?ÔVYAGNbll87GB 161814.7+554307?ìË<Ü
YÂ?«ˆpÇïI?—ý+—JÌG?"
<´–¬Z?³¦Î9Â~ä?¨ÇÚ`²‰ž?êG9©ë¤È?¾VOb?«ï­ÓP?¯O=R©vÆ?¿Î\)p?µ©€_ñ?í;`ÓZ[?•·<òµÞ?"ÙNâ·Ñß?öÕTÇMÝ?±.¥¬½?':К†úY?éÃ҂Ñ:³?¥
§òw§µ?¼Ç±}(Z? ˆJÏ"?µºÙù?—ýöµ*4FGL J1621.7-1103¿ïmJg'E@:RÖËSP	À9ƓX6ø»À;ò­×>?×@‰s,Û*@ÐÈb?Âz	2®?ÊÕÊw]¼@7E«I@r 
´®?ïƒ=lr"¿Õh'{Mz¿äœ»sG ¿çÝ]Ó6¿ïóüQօ¿ï¢æÿþÓZAGNbcuPMN J1621-1101?ïŠÞHû?š‰8"'‹:?pï»ÏŒL'?u`ØëOÉ?… §›X?–«°1\?ïK¤@`ï?'¹ÐOf?dæçïH?tGÉnï@{?"îšö^É?FÁOŠ¬?ìN\›]?£èDð®Ô ?¥Ô'9Q¶?•;+­xݖ?´"Fȑü5?šÁ΀'û¢?î¢Dïø?ŽwS/?þÜ?‹H_°4À£?wktŸ»KÓ?§ï£Ðf?ŠÜhãÉô4FGL J1623.4+0858¿Á½Ê>
h@BpJb#á‡À;a)ÄÀ<Œ«Ü'<®@ \<
<ç@V/Äé©|?È0§$G¿Qq±‰@4CºêÍ?ïü–ô£«k¿Ô톀¸!D¿ç|^?¦^#¿â?ü¥¬¨?±yÃeoñU¿ïÿÿ)@k*AGNbcuSDSS J162330.56+085724.5?[ïµù?‡ó5AP‹?GÒªšC?Nfu¶."?ˆ–¾Zq
h?†'¡âËãS?ïÍí?‹›ìôÌ©v?Jj³>?g,GF)?Ž"¬bîÆÐ?ˆ…϶É#?í±òcRäÏ?•Úkµb\?v4R"dm?g«Bvºé?±
'ÄV³B?"×!k›àú?îÈ\!'¢?ŠxXŒ'?UÑ9K7Œ&?P7÷'Oÿ?¢Ë´$ît?ŠÈýN—14FGL J1623.6+5743?ï€ÉÙät@EÅXdE$À;÷GʚÀ<ÝxC½@b*"y@ca	/T?ÃWSùÒ>|?"ãpäTäð?Ñóêî?ò*}'Þ?ïèÙ¨}b+¿ãC''%ο؉ }8é¿ãã'àp¿ë|'Biñ?ÇÈ?Il¶AGNfsrqTXS 1623+578?ï
iê¸5?˜"eE
Š?v3c'OJì?p™îTõb"?š1ÙÞU&Ê?–"ô0Ó;<?íxj€\K?ª›È`e?4?Œ/YI›Ñi?'n¡«
?°¶¿êÉ£t?¥ßža)I?ìf0ᥡ? I£Ðó¿?˜{qB;f?‹žHÑÆ/
?¶¯œ¢S´?š®ÜøŽæ?ë|[Á²¯?¢Hïá—?±ZË¢jƒø?œÓ9hœ<?²ÂVP?–V¬Bl	v4FGL J1624.6+5651?ɹ1Fkk«@E!©T!ÀDÀ:΢Ç?ÅÀ<Åð®{©@Qœ«qÞ?@	A=?½¼ËLïò¿FÚ«´XŸš@cý/ìð¿ï†'Ìͤ?ïŸà¥Ç¥F¿è6¯¿uÌ5¿ßQƒòÖL¿à 4óý">¿â[7(‹9…AGNbll3FGL J1625.0+5651SBS 1623+569?ïæ³ã${Q?`ÄÁ_§G‹?L½Ì=¡§?Fó>+Õ?b©Ìhÿ?Z"ãÍÐå?ï¢ëÝßOÊ?†žÔ¨cñÃ?Bð¤ãB?RÀ• åKe?†þ9úÙ)?…"*\s¾&?î4{­©®?TcrJÏþ?}–
HhŽë?l	Má?©,SE?‹ôŸzVIÈ?ïš\š.Ä?lŠ'ÜKí?sK"ƒ"?`©¿|Ž¶À?†eð?f÷i™Æ	Ø4FGL J1624.9-4210?y»œ"@1ßv½À9°\'¹À;2{"¶
n@é¢[	;@,üœ?Џ½ei?äý®l@Zw¿á?þÌL&t3?ïê4†ðIª¿Þ{?[µˆc¿èß6üìOI¿ìxToÃÝ:¿ïÿþó…õ?è–ý]
wAGNbcuAT20G J162458-420657?ÍRôWýrl?¾¼&†v?Õ:×ø—àø?Ç+@+ß?Ü­ÛieÓ?Æ3«+L‹x?¹ÄŽv¯?¼oF§§7?Ú?Ù´M1?Í}Kuãú?ßO¤l±=?ËË`8ã?ρŽ+5?¬PVeh?Уäú?¯@qj4?à:OÉêt5?³QåìÊ¿?¢à8-£ŠÁ?ˆdG½Š9ú?Ûщsn×Ù?·'(橧?àé7Ãn[g?¶IÛ4l¯4FGL J1625.2-3600?»"('Cµ@"|ڐî¢À9ô
 yóÀ;"Œ"ÎX¾@4ìƽ>@Ÿ¢È…?ÉQÄð_y?˛?áíEh@¤åýö;?ürµ"¡ã?ïþ{eÑëð¿Ú1/"‡•¿é³iï‡â¸¿çØ-Þµ'ƒ¿â¤C@Çp¿ïþ
ýŠúAGNbcuNVSS J162522-355452?Ïæ€\gD?Á_+nA?œ?2£S¾—?œ<{â?çZLÊÎH:?ÂaÖÌ6Á?ÔhÁª«î?ƒarÉÞ­?¾ü`Rçpˆ?¹ëCR/s?áìfÍ»÷?Ǹ²Fôˆ?ÛÂÇ' >?°
*SWW?¸Ä'ziH?œä(;Ôä?Þ6ÇÏ'©?¯'	"9}m?ÕÀ~ã.0Â?¥ñxõ+–ž?¾—j¸PÕ? ÝfjƒãÏ?áLÓ7h½"?©*;²	Þ4FGL J1625.7-2527?îÄ*©÷µ¯@0PÙÆ°SÀ7ÇϯÖÀ:ñq¤ˆ
%@JIOTQ@_3¡íûñ? :)­?Áªàú®‡@ n
ˆ~¿#@ —Œùù¿Ê"¸ç' ×¿áXß_vˆ¿äy`¿'F¿å(Ø0®µ¿éÜ°|¿é¹ÅÞñèeAGNfsrq3FGL J1625.7-2527PKS 1622-253?ï d
iæù?²1¨'Q#¡?‰Ù &åOg?²]œ¯¾?Ž
Ü~ òn?†é"ÎôÖ*?ï],"nÒ]?›}a‡Æ?g¼´äZå?€TI­¿§?'b黉)?˜›û:‡?ìxó¹ï7?¥¶ðï•æ?¦7ª¥8Ù·?™oäþv?°xc"o?žíÉÛÙ?ï)ºßv¾?ŒÝ;$#îç?båÎHVW?^j¨›g%?˜l»]d?Œù묥4FGL J1625.7+4134¿ï¬ò'ØZ@F ±Ù+€À9Ê"
qÀ<qºnü7@‹#IWƒ@l¼Á¼ÎR?¶¨åf÷…Þ?ÄÍï»õå@êiæM§S@bÜʵ›¿ß¬;W¿ãÜâąֿæQ%AX¿çˤ® '¿ïÿ°7ßj¿Ð¸âÓõ5AGNfsrq3FGL J1625.9+41254C +41.32?ï¨ÔÎÔ,?"µ.zcu'?yQNÕ ?|µ‡v'·—?rDŠGÌ?s©=üá?îßr*ܗ«?©xÉ
ùïS?lã'/ʑ?€~T…giÙ? HÏ#ˆ˜?§õ¸'$%â?îȨ™«Sj?‹ˆ—]E?'|åýSqå?zÿ™tÿ6?¬yËëÙÛ?…¼81 J?ïM'ê÷U?}";()Ûn?†LÎöZ?r2
#)^?†"ø~ª´?rLk£Ù"/4FGL J1626.0-2950¿ïÖ=LDYÕ@*§ïZ–N‹À7ö¿Ñ;ÇVÀ;O«›úœê@L;kæÙ@§"ÁÄO? æ……x3?Á<'§º™™@Øņ‡n@EŒê߇e¿È«]üµr¾¿ãS–JYÀf¿ç¥mB"º?¿èÀ;Yrb¿éüc'í"Ó¿áV[áþ`AGNFSRQ3FGL J1626.0-2951PKS B1622-297?クžóš?w|/Ñ|›?c‡Ôk
Yä?g>ø¶Ó?w_ÆPñ?q7cí?ï5æÈ"?›UËq/Ü?iÿÍ
¸¡?wÝ8\± ?–-\œ$½?™S¾\S3p?îL…u¬'Ï?™ùÁÇ4'Ì?'©í'ñº?‹ÔŠœg¬ã?¢b²!íZ7?"L¬§k?ïDÙ
.&?ƒÑi•ÂÆ?pë€ÿI?bpOæµFú?")îÿ¨Ù?ÕÞg	4FGL J1626.3+3514?í±ïÎ{ðß@Eñ&|k‹iÀ:ý|ªu‰ðÀ<±vö×bR@!)æڕl?öÀ;ú'¾?Ð$þÝ@7~?ÐR9¦j@qŸÝ€y7?þ½ ŸrK¢?ïm­íät‰¿ëU.enâ¿Êj^¼#¿Ê'dÜx'a¿ÞŸxkK¨u¿á´¶á(#‹AGNbll3FGL J1626.1+3512RGB J1626+352?ïYkßÿ"?‡8éíÕ©?déu˜3?_ò–fDú?'5U_ˆ½ø?"æ`bz¡2?îGrBNY?£R™ß~?y•,úýF?x~¸!¾?¨V:›ºÃ?¡1m'ñSd?í°G™Û?˜õ=o7¡?ˆ
ylüÑ9?x
øÍ'?´Ш#–ý?–o2,%)!?êO¹î»ã?¢
¥x4Å?uÈ_­?~\NÃ3"§?IJ_B'؁?¡õP_¿4FGL J1626.4+1820¿ï'd«Ÿ…@DãC0×8À:Œ"¦£mÀ<H'sg@u–Eý`@ÞûB0&?ÂhÁ_†M?ÏáÕ§?ÔM¬[==@ôB‡¿å;¹^Û؃¿Õ~àEO•j¿ì
c›°Ë¿áš«n®4¿à†FÁ—"¿èP%1€¬AGNbcu87GB 162358.1+182615?ï_*Ú ›?Šú´ab;?sií•]yÇ?m‡»Œ?Ž€R*~à?‡ª ôÔq?ïb&Ó]h?7‰Z|…í?OR"sÛS?Yr0yäy[?'±Æ8ø´?Žú®Y‡Õe?íwH9`ä?•¿aF#} ?Š)êÛö8O?}ñ•,®}?±€ÜV1Ù?'±qÒ¡ÕÛ?ï# ëž?€ö¥Æ2?núÊ*Ė?_üõ,Þ¥?—¼º‰FçY?€Fà¢^½4FGL J1626.6-7639?ïÁ±7'_áÀ2͇+À:Ba¤`À<Rmý3œå@ /ù€_
ý@LÓi©?·b>
¬»à?^ê8§în? ˜‡Üéá—@	xš¶O1ì?×»©äÀ^¿ÊDAùI­¿ãqøjà¿ßŽÞ	àÿ¿àúÓOÍ¿Þž6œLÒAGNbll3FGL J1626.4-7640PKS 1619-765?ïöµ2%Ð?K͏s¾]?%,4HÆl? ¨[sd/`?Q3ð+D'?Hüè©<#?ïÎ/¬®ƒ?{ÎÓÃ!À?'–
ýÕ??Ÿ£²Dj?x0A(NÒ?{
ͱá¸?ï&-†´&´?€0e"ȓ?cÞ8Z?Uµ=¡ß ?˜¾ˆ&^"?~"áΑº1?ïqi15ö?tÌ ⬒?bŒl$Tg?MúÆu"ƒ¦?¢î)m>?t\cs†b4FGL J1626.8+4337?ë¤y('L˜@EÿO?Ù3ãÀ:ÏÀXJCñÀ<Š¬®IT@ÀjS†@g@€ù?ÈQ:€Y'?²²"Ç!è?ã±2!»;«@îOá¿£?ï¿}X›M¿êB€x`cî¿ê×¹Z)AB¿à£Ò¢Ï£A¿ïþQ€ž¡¿Ï•½ÁìôàAGNfsrqMG4 J162551+4346?ïΈtŸ·,?}LÅLO˜?t&b¥GÛ?{Š8*O¡q?RUŒ+uiÝ?W¾n×|?îûžnEûÉ? ævÂ]´?ib‡Ÿ—>¥?€Ò2 0?_áCMžÌ?žáÊ$ù9?íïþÝF©?'ÖL¼Œ?ƒ¯mUIª?såHY_Ûí?¬H¤6ÖC?à-êg+?ï`»ÎñÕ?}Ëœ˜TÄ?"cE Ûsn?t²Š9Q?ƒmÆÜè?oÁUÛrë4FGL J1627.3+3148¿ÛK4æUxÇ@EŸå\ËOÀ;
ÿ'E7À<ªmà®+!@ ¨7F=Q?÷º›<1·?Ò×Î]›'–?Ò¹C£Bå®?ôJ…) z@ò‰§ß®¿å—O§Ýÿû¿ÝÔëŸuѓ¿äàNjDlA?¶g¡	$—¿à
¨à"Í¿å¹êqùA AGNbllNVSS J162712+314954?ïü^Yø?'±8ÁmÁE?h'—¶³?`¬ê—»½®?™nLý^^¶?'…Ôçro<?ïrÇ¥ª—?Š²ƒ[‰•z?Kï%
²¸?^ŽYM·?Ç¥C"?€?ˆ¾Æý›Ñ'?í²ÐÓO ?Ùïâ??‡%'ß¼áO?vf`l+*N?´5·mêÞ?šúŽ#F?îWIÞý˜K?'™0˜?e{ùQ€.?_á‡ó¡0G?©3¢{#D?ŒÏ…^ÐÄ4FGL J1627.3+4758?æ,nÿ£J@EƤ~Ïé¸À:вýî­ÈÀ<™M߆ã´@Ÿ…@ò
¤@Ú`üšò?Ê0HÔÛd?ÏYÌ9©ïÓ@¿<pɖ·@"¹D8¿¿å塄õs¿àÝ6aé¿æbEÚÕ¤¿ëd¯­Uk¿ïð¨ÿ¾Ç¿é	lLþAGNbcuMG4 J162750+4802?îáJ¹~#?™‰ }kè?‡d•eýf?‡,9‹¿?˜$'}=:?""–'±"?ìïâ@ÕÌ?®\Q¹:YD?•m‰p…0?—Þ 5Þ?³ £0_?§µÉQ¸ôç?ëí
³¹t?¡Œü¸~4?£qmÀý?Ckë´?¶Þáh$ã?™ˆ:š¡[R?ìŽ/«_á?™gâÎV?ªÜ¤ðix6?"yúF·Éá?¬@`Y¥ùÂ?"1Ge…4FGL J1627.4-3301?ßßÃDʊ@%ëßm¹@ÿÀ9ÎÌ¿`ÓÀ;Ž1á#›æ@÷âzÞîb@BVÃ[?Ä¿4žBJÓ?Æ«:ÖÀ–‰@ÒÌ:֕£?öÙ6Âß¹?á¡èˆ6?ïüÀآĿê´k¬÷Dp¿âi`Kš2F¿ð?ïÝüÀ/…AGNbcu1RXS J162725.1-330322?ãvÚªgû?Ç^õ÷ÇÝ?Á
­.êCe?¾ImUù®?Ќô¼ÄX?Ä^#a'Ô?Øps¡‰©?Ð ç´)z‡?Øoò#1½D?ЫˆiÙý?Î?4vŠL#?ÆÃsþ@ÿ?ÝZÍp	yw?°'¶úÐs?¿T¯j±Å0?¢é8֟R?ÚеJ;?®´!ÎÕÑê?Õ´W‡+?µåY†E?Ö+RÂß?¹Þ:ó?Ô Ÿ¡p?³›y®†áü4FGL J1627.7+0251?Ðötª»š@@{ñA [ÀÀ:" ‰ƒœÀ<o§yV-3@F‡"^qO?ýŽö¨hi?Îs€?ÖY¾?Ò"¿µî?ÿäùdŒW@	âe£û
¿å	%B°¿æ…ZýýqZ¿Ó77dENê¿á­š'w¾þ¿äÞ><ü‹¿ïìüLíAGNbcu3FGL J1628.1+0254CLASS J1627+0251?ï‰Òg_??";*îv¼?Rà‡ý¬á¯?L	Íðxã?‹/U(zœè?ƒ4̎Gƒ€?ï‡Á½a'?ˆ$ÏéXlh?I¶ˆ'–‹?Xe~ß
?Œt(&'•?†¾ó–@u?í7Iºvph?œ~ɀ͎?"XÇE/t´?†'@¯Yê;?±o€[ŸŠ?—E¢ÂåßÐ?îÛ{G?Í~kU"‡?c)òó9Pß?NfaÖø´?¡¬_ªº?HžIÙ¯4FGL J1628.3-3343?é0Η'Ny@$±·|¯ÞÀ:ê#èùÀ;âo¼h@ Y¶Âs@Õþ¤¶-N?¾«>‡¥%i?';|¾þ"+?ÖÊû>ÊÁ@.d,$v?ïþÙú²¹%¿ëb†÷¿â‡k>gnÏ¿Þ1œDÄ«¿áP·b­IO¿ÓW<½J£½AGNbcu3FGL J1628.1-3344NVSS J162819-334342?é 9ÀW¶õ?ÁCœåêRC?~!ÿú†Ð›?tÏpªc
¢?ʎþÌíª?Á†&=¤Š?áÿ¾_õ?Ȅ€$¡F?{8†ª@x?"{̲¼\œ?ۓ¡(
Æ?ÈZÝì\V?èh*¼©7‹?­ŸÏlî
3?™eŠƒÞÎ?ƒùÏè·@Ý?Ë2£¼ßQ˜?«É«ä8)Z?éÎÜ˽`? %¢%HNï?'ª?vy›S32?ÆòÖË¿ŸÚ? ÉáêóÔ4FGL J1628.6+7706¿î#Пó®l@A
[–(ËÑÀ9¤š~›çÀ<,žZÉz2@H¼áGX.?ÿS‡œAÇ?¬ß¾¥Ð?·mÅÖ8†Y@
Ý®ˆ*Ü@…í
´ôi?ãþC›`C¿×û=j¿à8@¹-³—¿á­ýžü¯é¿ä"q`¿åò"šCäAGNbll3FGL J1628.2+77036C B163030.4+771303?ïàíNÓm¦?eÛ¥ù7ª?<M'Ø­"?6–h'Ù?k‰Ñ|¨Î?cãv6Ë?ï¹,þÌõo?}¢NTkew?A¹Çù¡?W®ÜÙe¿?€™([$}?{g@)y_?ïÆõe|?"&T1[ö?y˜Ç‰ç;Æ?tb­Nµk?˜ ïpÖ°j?~DßÁiL?ï܍¡®â»?ZI½˜¸z?9g±ÑËøX?)K¿t?p"´qât?YÓPæ6•4FGL J1628.8-6149?ãÖßȼÀ"a'ÚÀ9Z귙^áÀ;³ÙésÍ@Ÿ¸7"kÝ@Æ[ê¡õ?µ›ƒ~¥!?Ϫw¢Î́@"ƃÝ@ã&q÷?Íî´(;2†¿ãf…·æ¿é|¢èÍ´¿èÝíPÐÒì¿ì̦×o½þ¿ïý9Fr«AGNfsrq2FGL J1629.6-6141LQAC 247-061?ì<EøÊÈJ?Ãl@Ý㢰?³êÈÒáл?Ã=Ì=7?¤f͏Ùá? «ß3µÜ?êäŠz³Ø?Ã*	¿.~?ÛQ«0¯r?P"l¨UÂ?ÃQì»b%¬?µ¼7Ò*?ëmQÕk=?ªÚ_ª›c?±—ëžÛda? UhMQü=?¶©ÒyA¸? î ‡²mµ?ì3ÌüX¤k?›}q¡wè?¢øßj_óh?‰¨ú›uÞ?´å(h
âó?˜ß- ºÒ4FGL J1630.6+8234¿írUB°1i@?:kÆ!·áÀ9
¸ª*À<&VÁ­´Ú@Îæcæ"@²>¬
:?¥ž»AŠ?¶Ì`@\'{@%äêÐÄ?ýTâƒBj¿±yƒÿæ¿ß^謿ä¥/š!~Ö¿æB• Ž¿êÛíÒt¿ç
'Kº"AGNrdg3FGL J1630.6+8232NGC 6251?ÙàŠr­Õ ?Å>1S'ý`?¼Y•´"?²A­ÜÕFB?ß	IO=½?ÆZÝÓÈÎþ?ڟÊÒêH?Ðï'þ¥,?Ü\Š˜¾°?Ñ}õýÚ½c?ÂU(®Ni?·¶2(ýù?䎠'Öèb?±³++Uéz?Ân3­¿?§6	Ó^ý?ËWJ¦°´?«ë
™ý?â<Aê±¥?¸ŽëP¸?Ô´Ú'úÊ?¸j^Âéêy?½û@&ì?¡ 42Ýæ4FGL J1630.7+5221?Òd‹?Ž¶<@E2\'ÑN<À96Jbú¡À<Ãõ¶7@G¶¶_øä?ÿ%"Ùîô??¨ø%
?Ž?¯Tkì @Oäë8@	l,¨T¿ÔzÁWÁ¿ÞÚÙÕÊ¿á*p·"@¿Þµ6˅…¿áÝù ?{¿æO6WªâAGNbll3FGL J1630.7+5222TXS 1629+524?ïšÅôE¢Ö?‡Oi'L?P÷«Ý(d?N"ýÖ<'%?‡/rò=æ?†R^˙ªä?ï;l^šo?›ÉmÀ"?`쉾½ã?m
Ս%?–tâü¶zy?™×MBîT9?ï1ûÚ%?‹Ü;vq?oøWÅ?a9­'ї'?•ßå°y#?{ú{±8?îð…×l^¦?'¶›¸a»ù?{¥Û¡†˜?c-¨-W?›([›‹É~?Q ëގõ4FGL J1631.0-5302?ëª[™êÞÀ	ú D®…ºÀ9›)"N>À;3+­,ô@
fÑ@OÙâ_I?ÉÏìçÊT"?Ç¡¼}Ê0:?ÿÃ¥¦î?þ,iˆïú?ï—c"$ӿ犻°DÖÊ¿æÄS­úпëoÖ½—'¿É¥ì8Lø¿ïÿxáh:QAGNbcuPMN J1631-5256?Ð[y$͜?¿±Qw½¯³?'¢ ðP<?p
‹ªÞ`?çmA;鎱?ÀOõ€‰&Ó?ÒÕ·÷àR?Äz-ã-ÄÆ?Š_ûǽh?"!†ü5à?æ+¤ pá?Ä\"ÆBJ?×"n

`?°T΄ˆ¥Û?´cŠ*Än5?—ײ¥¸3h?áåLƒ¢kŠ?°}*d>Ɲ?×Èj	¬?µDE_ø­¸?šýçÑpÎ?_4U#þ?ã »Û¸ï¤?¶T
ʳ54FGL J1631.2+4926?ÝÓû8€@E`GýœÀ;$›À»GÀ<¨a¦
Ec@O+†®@ëU¹oø¶?ÉÀˆÊ>}?¿à¤ø?òéÆؗ?øµñ–°±
?ï*u¿á+3Šq¿í'ÿò> ¿Ç×ϊAaõ¿ïî¡UЗ¿ê;+ðHÒØAGNfsrqTXS 1629+495?ï'x¢~+?˜otöòâõ?}IñaøiŸ?{àJ$ŒŽl?•4"2 2?•Ú;̟lÌ?íIJ¯?²úãK[þQ?˜ÂLC "Ÿ?£J¦¶%˜??±'GY¿B?©"¿þÍS
?í³{t%?šÁ0ùŽÜ?'žûÝ.ŽÄ?†oµCå?²â¥-3Æ?–»ƒO\Y?ê×=€˜Q,?«Nkã	!?¹Gß=W?©S\Iéá½?¯üi|t¼?•ÃbÐÒÜ4FGL J1631.2+1046?ÌU®÷éu@Aü¸{Üð0À9ÌöÕ´ÒÛÀ<&ç­"ãZ@0&îV_]@->" 
Q?¹ñ:j_k?Á!Í°!›@^¡£SW@ÿ³ÿÌT?ïýZž²O¿à‰xïÕæQ¿çYߥ¥^¿â-¸j?8û¿í;‰]â3f¿Õ:Ûs-ÊAGNbcu3FGL J1630.8+1047MG1 J163119+1051?ï'¢Á[Ô?'àør!œô?{öSôðŽT?x¤Þ"Õ(ø?•Ðª˜aò?;[e7UX?ïkïÆÏP?—žï¢"	ª?oR´ÙK×?y»B†!o?›ˆ+kü²ÿ?"$Ÿ3Ù?îÎÅ",^¼?‰õÌ*:?€½æ‹?y"(þDCí?ÈѬ Ë?ƒþO\5Úé?î#ü-¸§È?‡ÄÍã@Í?š7‰ƒ:ÃÈ?™«7œ? ¤xbØ!¢?Á÷y‹$t4FGL J1632.2+0854?êó·K–@AuT\x¦ÛÀ:7,ÅÇÀ<Eq±ôr@qjKÎ4¬@*"³‰.è?ºæPA
$?"'CoÏ?Ûå'`À48@
X!þ­o¿¾63Úg?¿è(ÝnÛî¿ä+3Šq¿ãg&f¿R¿éïm«Õ€?Œò"‡$çAGNbcuNVSS J163211+085608?'‰[Á?•Å?E.?gKd">Þh?[gú"¸ÿ?…¿|™XE?H@î¥?ï¬ßxüM2?'³PÀ×Ç?B™g3îÚ?Tovõo¼?ƒž‹M­Æ ?€õ䫂s?îçH½/x?‰_>ýL?tà\/}é?o´§"&Ç$?ÞöñN1|?…À{hÆ°P?ïoô©
?uÉ=Ö?eP2I"®µ?QsÖÊ1¥²?Žä6Cpó?tK÷j~ù4FGL J1632.4+5800?ï!÷Ø@Dzl <K
À;Ҙö«;À=µ?è@ Æ*ÚI7,?ýPaâs'??ÑEZ}$
?±‰Ä6Š?âi¿aTXÈ@Hñ0.q¿æ7­wa¿î-Ƭø/¿ÃÚÓÍ$á¿ã@9¿Ü0Ý£3Ì5?"gâèB3AGNbcu1RXS J163213.2+580109?ïˆB~‡?vNÿܞÂ?/°œ(w¬?(ß""6|Ü?}¾Zûßyb?uïꃑ&2?ïMÚÃtê2?'¨êwYø?Pêm¯Ë"	?cÛ£ú¼?•6¶fp?'"LˆËx?íÈó>Е?•±Žª`tï?vb>>¡<?rœ¿CÎeÜ?°RB(÷'F?"y'?ïËÚ?ïƒt_=¼?|ÚÃY'??‡"É?9n¶ò¶?Ž*š¯ëïŽ?|íI­óÕ<4FGL J1632.8-1048?㣃‡«Ó@8Mqâ›k+À9Ï0âöÚ½À;ÆQ°Ì¼@),P•ï–@Z䢬gÒ?ÂʌU¹E?Àɽ£ºò?úTâ_ܪ@"šÞ=7™?ﯷjdù¿âº¾ý×0Ô¿è';2ô¿å¶<'gN¿îŸ™Þb÷F¿ïö±½|ͱAGNbcuTXS 1630-107?ïØzÒ‡)?ˆ÷"ÙHÂ_?TÞUF•?qœ¢‡(z?m'€é´¾?€Òk[™Ô?ï³î(&Øó?ƒà‰•ã¢}?@AÁ
š?Pàf[²ì%?'Yå©?'Ã"ˆ6l?î@ÅÖwœ‰?"àcÀaô?‡g¨Õ"a%?€ÁV̘—?¦¸c!_"?vÑD3{?ï­vÖéâ?lt'gõø*?PÆknôšì??…ûЫ?'‰'fóâ?k=<ùe4FGL J1633.8+0701¿æÆK×w~D@@Ú4üaÀ:>*ՖŸêÀ<QÑææT@<~"ÛH@½'Óh'?¿XÊ`OºÂ?¶ÿ¬ž6?÷vÙ˸З@	'øŒn7ì?ïŽ!ÛòÚ¿º½¿~/°È¿à©(ü¯i¿ánÄÙ¹D¿ä÷K[H%3¿êÇ/~ó¦AGNbcuNVSS J163350+065705?ï¶97MÍ@?}ŠŒÏñ!?O&ôÂã?Gæ_Tä~?€EñLC²?{n- ¨¼–?¯äÂ?ˆ~É5üY?RìgU^q?^mq!ÎIÎ?™Ö°#Û?†'~¸ºÑÝ?ïxuo­¨?~]ŨVU?mªol§%«?cG\'AR?˜{£dufh?zcèëó¼u?îI}]Aš?…\Zd‡LÄ?†Ì¡ºþ?j¶CF¸/X?¥á©¸½ïj?ƒ˜²¬Ú/¢4FGL J1634.9+1222¿ì…û'ñ@Aé4?¢­?À:øÓêÎ?"À<dInÞÛ@ #4ÔžÓ@(ã«5£?»­¢e6¿¸>Ú 
ëÀ@‰2"Ѽ?ûž"Ør}?ïûlb&¿è¢µ6®÷¿ã #Uož¿îû9Ç¡ê¡?âòc"úÎh¿ðAGNbcuNVSS J163502+122142?ïÁÄpX?"·Á¤O?KÇy; É]?SVÀ,¦"Á?{¾ÈvSºŒ?ƒ%¾ÛÞ)?ìÞê-Q]?¿"{Ð
a?"?Ði"¼?©#ÒaÓáµ?³øºy…ö?¹ÕO׶t}?ì©eY?›µpòàž?K5./?ƒ	.B"‹?¶¤w‰²G¡?˜bãlOº¾?æ}˜õ}º?¼	ϵ››?ƒ¸émö£?ªtU·&Ü?Òg|¨"Ö?»˜‡Ê£/j4FGL J1635.2+3808¿ÅbÃLNé@E*â:¸cÀ6K¯*ûVÀ;	ÇÿÞr@Ÿæè%@£$\֚¬?"}Y"M?ÀMfûŒ¨Å@4 uĨ;@!›fçÀ™¿ÉTå ig¿át·AË&"¿ælÐxR÷õ¿çP¼ R;¿ë·
è`Ý¿ïÿõïùAGNFSRQ3FGL J1635.2+38094C +38.41?îIå¶*;ð?©œG#Û
"?œâUU¤Â?¤ÈjŠl	?š¥fåbÝQ?™_¸v[êà?âk£[:¹)?Ùø¡à‰ì)?Ö;¡¶2»Ž?ÙPÌ¢½Î?³´^M_H~?º™-œE‡r?ëƒh2b?©¯2ÙhRÌ?±¼ÞY³-ê?¡Ÿmìoݔ?²*Æd¹Á1?£tÄ»1?âÎå¸ö?Ìj.¦³?Ў	#d'?DZ¸³µrN?èc	àڄ?¼>¸è·í4FGL J1635.6+3500?î–ˆB.N@Dü¼œÓà½À<¦-%ÒøÀ='ž>Dn@Õ³¦53@÷C˜Ü?Údò=I·"?ï*~ŸBP@.ðþÛ<Ò@Çy–™ßæ¿ïqÞ?ïýnŠø'¿Á‹½ãÐÊ]¿ãàâΖÑh¿ïÿx@XŠ±?å(@[9âzAGNbcuMG2 J163505+3458?éÁsmíOè?Áí!
U€ï?¿ªœˆ$u?»k8òn?²IÈq ?®ª¬%H–?ãc²­_˜±?ËT|ÀK·¿?Ð]:¶R>p?ÉrŽ÷~?Á¶¿ÝÝ [?µÒ¸+dÛ?æj}E?±9§€[?§öûö*²?ª8B1?Ã_õÅI?£ùËV™?ç¬eÈáÇ6?µâ6U
?÷?ÍMùN@è?µDš…fÛ? ¾8ã?"{E"-o²4FGL J1635.6+3628¿åÅRó ~Ä@E"î9.À: á$r¦À<	t"&"@wæ£ãt"@ë&T' ?º0@åxjJ¿ªµèž~I¡?ënþ…¬|Ë@ªÖÍvì¿æM˜9GIk¿åcÉ2äXÛ¿æÞ£ßm¹A¿äõ'ÊIdοïÿö$´ë/?îï'Á8AGNfsrqMG3 J163554+3629?ï÷+pW£"?ej'¹ûC?EJ%= DÄ?_ÁWÇ?<2È¢Ï?Hí½¬b$?ë¿I?œF»äû?=®÷d¹,2?Qsm_äq8?ˆ²MUð5?›ÂGæÞ°Ð?îÑ~BÖg?‹Ÿ{¥'è?yH¸ÁIj™?oìw}
ˆ-?Ÿ~‡RØ£?ˆî­ºØ?ïå6ÑÈìk?Z_¨œ›i?-¡qê`ªª?#'ï«¿Œ?hïmŠù?Y¼R6|Y4FGL J1636.3+7128¿ï|ÛÆí"@BbA=·ñÀ:ê‰Ê½fÀ<šlvJà@G`Ö@r$'–GÖ?»ÆUˎ‰¿¾4b2O2˜?ýûk{y"@•àZôi?ïøf–=ï¿ç_·ö{ó¿ëô(üxŒ¿á;Þ}yR|¿á@W¥ÙC¿ïÿèã«6AGNbcu7C 1636+7134?ïž›ÞО?y;"oÞ(ã?w®ÄhïR?v3ƲûÝ?XP
0»ü?añÕߜ89?î±ê"rÞ?§ºÅ˽)é?z.@n…G{?¡eü"2ø@?¡›•Ëvü?šÒHM׍?í³‡Tí	?•µï}»??‹¼cçºc›?€ÍãJ$ä‹?­Øq·@F…?"-q9®y?îŒT€?')ìu#p?gZ;ü??ƒz
B}(¯?ŸÁÒß&b?ˆf,¾s4FGL J1636.5-0454?Ô_Àá:@:óúã`	À;"ˆ\ÙöÀ<XùD$?@!ñ¨Ôõæ?ü—ù1~'?Ó3®BÈý_?¨$ j»'?Ñ» |ø#@G6·!>ê¿å›¥"
ñÛ¿íàœ…˜?ÅYGŸœ¾¿æhãï(Ah¿ÑßÇ[Ýá¿Ï…òGۋ×AGNbcuNVSS J163631-045506?ëÛ²¥aa?¶Hw
 èl?\ìóíSÈ{?Uo©"†5?ÀW['ŸÒ3?¶-ऄv?îŽÈÎp	²?¥¬	p
™é?iOLp±(´?w'ð	–?¥~~QôR\?¤˜ÈÕô[?ìÈd¤ZzV?šåHi¸Y?|̗ªÈw?m¨7{?·ðk±€Ã?™Çdg‡Y?éۗöÄÎ?­ã#Ïyy ?ZøQ5©5?Xc'ÀÛ?È[³E'v?­ì–™×34FGL J1636.7+2627¿Ðg™öÐp4@DŒÁDŽÀ:Q÷·\"@À<§".Î@âPÑQl@ÉuDO»)?¾i®oišM?¹
·ß»øû?ûŠYUëÒ?ùgÐáÚP?ïþ˜â9›'¿Þ†#3‹É¿ã<b0÷š¿âgpÛs¿á³´,ÂÖª¿ïëÿÝÆDHAGNbll3FGL J1636.7+2624NVSS J163651+262657?î¡f'_*?š-ë3|]?qZ'?ÕÙ(?gñŠ€0Jß?£¾D–ORD?˜Í; ³?ìJV¢ Í?³~OUÞ? í¥4ŽFÜ?¡C"Äñ?¶žÚ°§Ö-?«õÌý§c?íQ
-é'?˜*¾sÇo?Žÿ¶þ·=,?€`Dh‹FI?±—Ÿ°à\D?"rØ0EÉ2?çzø[D]ñ?£7!ú¬'?¾@3TàË?œÉ£1К?ÂôùD×?œåöߣú4FGL J1636.9-4103¿ìBlÚ|ki@€ÙÃUTÆÀ9zþ‡YûõÀ;)'o(¬Ç@{1ÊÓMo@Æۙj?ÈWÔþ©c?Ètè_Op×@òyÝ;¯Ù@ÊsѳçN?ïÿÖyô¸¤¿Ã¸«Ãã¿èùD$>û¿ä?˂þž¿ç|éàƒãпïúšï°AGNbcuPMN J1636-4101?ßø0®(B?ÄAmõ[5ã? 7ixôaM?®#)ö¹2Ï?Þâ"ÝK•?Ä<¢ÐâæB?ÍÊÑ^.ñk?ÀZ¿Óšß?À2Õt?¼/Wη•?䇾ó#d?Á¢ƒù»i"?Ø[ ¨Ï?²ÂZ·£?µéAÙdd›?–ÜUç¾S?á*4ɟ?±¶!ë?g?Ï6{ˆ?Ä?£¸ƒî(m?¸ú¥èIË?šmÒ¹¶^?å`çí?¤Ðì:'jç4FGL J1637.1+1316?Çóàυ†4@AÚ!xöŒÀ:úmPes!À<sÝo²?ƒ@SØæ
¶@u ÝD?Î4rÎSµŠ?¸"éclâ?îD½¿h¶"?üÛr<2‹C?ï³hëÒ¿áúóPÅr¿ä&Iàô¡þ¿Ö놡D]Ó¿êàˆ!ö¿ïÿý`éNäAGNbll3FGL J1637.1+13141RXS J163717.1+131418?îH1ÿÙ5m? 5;0ÞÜ?r¤Ó+m±?n-µ†'~S?©(E¡‡;x?žêQ¬[w«?î,$,Ï?ŸôÅVÞÂè?}=ô2D­z?€Âa†‰3Y?©–†êyî?œO­ìo?í#j@¹©?šå…¨¡Á?‹+o£?{ƒv¯³=Œ?³L¸Ò6?—‰ø
éЮ?éÝ:KX? "쯃3¦?¥®˜8° ?Œ'åé®]ü?ÃJlÅ~v?žî€E`§Œ4FGL J1637.2+4327?å¡+§ß¾¨@E
ÆûÒsÖÀ;ÙPVY¨éÀ=y_gn¤@!'ïCš3?õA³(¶Ø?â`€É>"?Þ´Ù% £y?ý	µU·Âz?ìsö™Ïտߝf'Ú?ì8ŸÎz¿Ø"€ð«N?µÊ£QÔ3¿ÝÜ°Úþ¾·¿å95Á-sAGNbll1RXS J163711.1+432548?ïX¬Ù/â?¢fJ(Q'?'Ź‹ÒJ­?‰RA~¹}å?"'
žðÞo?šþc‹'«m?íj˜ÓY?°ˆøuö |?"áJç4±? …ïìmFM?¯eØ󈾕?¥.êÆz?ì'IR¨ß?¢ç=ÀÍŸ?—Vžü´ßœ?ˆŒ¤e?¸ñ¥ö=? é:Àö@?êt^ÙáØ`?ªâÈúS?—ðX[¤U?™kÄ?ÿ
Í?Ã0ƒm)ó?¨aãMI4FGL J1637.6+4548¿æ7£Eûóè@Dý\B 6À;©%ʔä(À<ùZ'ó+@!¯…>BÜ?þ¡YKË°m?Ëz©u¯°?OöìˆZÖ?«¾œ!M€@~3ˆ˜•c¿ïÿT•Ð·?ïÉL¯Ûû>¿ãÆ'+½óì¿éC•ìeïH?ÔÉJ àuK¿ÛÈ…3[!AGNbllB3 1635+458?ïÔ²ü"'[?r¾òWj?>*œÄìã"?Bo´ôè×Ë?sÃ×ê",?pùºS˛ñ?ï…ÇÌ´›?"‰=æ­?E§ìZ¦??b¸ùžz?3"Đg?"{¬Hx?íÕ>ÿ¼ý·?'Dpq/¶b?|䔛¢N=?tÛz(ú?¯}p»ÚÑ? Åÿ<¬?ïv
·…m%?€ôî>SD…?Dµ?EJfErëâ?žCg%ó?€ûc!@îp4FGL J1637.7+4717¿Ø<Ý\x7/@DðÀƒn˜À8Þ©°â‹À<Aæh2ï@LtQ‹è@,Âþí±I?¢RFýHY?¬&|w"@¦#×þ@¹Ûÿð'¿ÂGpÂ_ág¿äv‹AèÜ¿æ8o'Á¿åM
švX¿è!£=Ý0G¿ëZA"õÆAGNfsrq3FGL J1637.7+47154C +47.44?ï¸;MâÑ?…]WKæ«?F©aó÷¢ƒ?AŠÜò…‰?€"
GÒ?…8÷tn?ï'Ë ÝEv?›ª¢ðö,?I&«Çç6?\è €Æ'?º­00à?š|¦3ì?ï3ã$æø?'™­õ0ÂÇ?l¢Œrq_z?a§^^'å­?–²
õ
?€üɝ
Âu?ïû'P¨0?5Ö8~$ö?&¸°À*°?±¦	ː?;xé"^_è?2ýu9F4FGL J1637.7+7326?æ;èʕv@Aœa|ÚQÀ;»`iÍ#4À= á÷×=@ ÐåZ7Y?ú̓ÜÁ6—?Ñ&Ÿ|¶¨?ÌßI¼ŒÂ?ùñÅû!sî@g°'£#¿î@5¯å5y?ïÛù%k¼¿á2:DŸlA?Ää^ú6gp¿é–Š ØR<?—çCp˜AGNbll3FGL J1637.8+7325RX J1637.9+7326?殺·uH4?ŸæFCIŽ?k?{–ŸŸ?VSU‹l?‡æ·•§?'¢¶§M?ï¾+õ¨´d?W
Š*]?<ë_3(²‡?Q¥ì/T)?O8sBÁ?€@ãԐtð?î`:ғ?"²Õ%Ê@?4h‰ßiº?y¦Õ˜Q0?ªüâ<šüw?"‡Í¯®\>?ï՛üUԞ?bŒÑ/lÄ?LÞ%þ¯úÖ?B9žQQ»L?q–=?±£?a Ú_%w4FGL J1637.8-3449?Øh…íaº'@ L׌CoÁÀ8ì=áâßÀ;²ïQ/@ h½1øv?ý"
¹&&Û?°?lÒf>Î?³a(c÷KQ@¹üȽ@ŠT©$¦þ?ïìæè×ÅN¿ã2´ˆ2i	¿ÜÀþè(¿ÕN]Ƅ´/¿à¾há?öe¿à2ö—¡qÕAGNbll3FGL J1637.6-3449NVSS J163750-344915?ëÚ$³o!?±')é|ÿ"?dÜë[pÁ?ZŒ	+Îìß?ÀCûûÆ9·?±o£8Þ´?å˜
à?Ǘ{ÀIYl?…œŒÞcÎ?'Hähe»?Ô'¿ßØêÁ?Ç=µCdïØ?ëÁ*ÁÒN?¤KͶ®$ø?†Ô^š­Ä?z>ÁóºF?¿(%š9²?¢Ö€Ú¡è?éªËBÛ?¢M;ª]Ü?£¹
·™œË?†ÜÂ9F?Ƴìa? m¨p+eç4FGL J1638.0+0042¿Ö¹3<îH@=¦ë¢zé«À;-¸éÀ<‰¿1×@"(Z)ÂC?úTœ×%?Ìvì…ú«W?©T"¢Í±
?àÖJ>ès@]/Ûæ¿é««Ÿ«y?ïÿY²"ý[¿èöÝÂhp?¯p
BèÌ¡¿ä
Cë[r¿Æ¨Ã
†AGNbcuNVSS J163809+004223?èu'Ú?(ŽY_þë?A±¾£æÆr?6™ñÇýÁ?Š9iø`Ý?€ï9%Ö
?ïŽr6š™V?ˆ^ñ€º?Hb­"ú£?UIS*>¤?ŠÝG‡7ÊÕ?‡Níxö?î6ûÈSl?"ÓXúÛ?rV8´?\7IW(ý?¬ÁÉ@¤9?–ÌïtC?ìhm%‡z?ò<üo05?"SÀìF?{@ü[H±Ü?º;ÔÇs¦§?·{×½Pš4FGL J1638.1+5721?Ñ;
Õ=@D/ŽèÀ9Í|ÉV À<†ŸJ³'y@;Y:Æ@Ü6r?±¦îýàQJ?³
è³³ ?übÏØðÇ~@°ŠÖ2Q6?ÑÓ-äê¥Ñ¿çßÂ=&Ñü¿æôV2ì¿ë
`¬B"¿ãæò}`}ï¿ïÿ7J³AGNfsrq3FGL J1637.9+5719OS 562?ïî·Ä(i?uªZPªÄ€?=GBãˆ9?U{«Z¾y?\"~¦öLô?p™™ä ?ï4aúz?'±ÅâBçš?C®?ÐzÍc?S6_ù´äB?Šø"T4Ë?'WXú±Þ¾?ï2¹w§?l*¼ÉH?n¶°ážÀ?iî)S£zò?•æÚGó—:?}°¿Y·ûš?ïâÞ£
(?UÈÎùÿ?ZgñÏ,6?J}õĸ´?_Ûì꿗?L˜÷þ€Ñ4FGL J1639.2+4129¿îhg£Zì@D܁Ü
²pÀ:^þُRïÀ<HKv @õõ0Ä@ˆœä§´å?ÃDuû°?Ðìà=—æ@
ί%@8у?ïþ@bEÅ\¿Ý݅íjñ¿âÁ}
q؊¿é!¿îB¿ëK¿Ê߀ƒž¸AGNfsrq3FGL J1639.8+4125MG4 J163918+4127?íkŽzKˆ?±¾×Ë5?Š›S/{W?ˆãùH?´¡@Ç´T?°GÛ}5c³?îë[ÉX¤"?®ýfò@Â?d™½Á)g?u8¦É1˦? §ŽdûJ?®a>Åﶲ?ë; ãˆØ—?¨DÔìHq?«»ùPÃ?™L©Lø?¸Itg3'ä? aÓªF'@?îÔo˜¦U=?†eŽx?tò—ó£©?c:9šÃÜ? ³w&Kö?":¥a?™I4FGL J1640.2+0629¿Üü͟ÊO@@*Ã") À:º$§5jÀ<f®ITè@!P5©/8Ó?ý}<9Aj?¿Ž9ø¹¿r2byíŽ?´; C¦7@ùùü/æÍ¿èÈEßÞ"?êBÀh Ó¿åù#7<­/¿Þº/(¸¿ÖoïœZ" ¿Ô1"\p™EAGNbcuNVSS J164011+062827?ïr¢ím~?‡2'wx~?TµÒîôè?OGX¤#%¡?‰b`ŠFÁ¬?…Ífñnñ?ïd›9o³?‰]ÕÂߑ?MvɓWt?W×ù/B›R?ŽOl˜n¢??‡…oZ¾6Õ?íÝÑÁ¯d.?'Å÷Úw—?v̶èj?a$wegþD?¯Ic®,º¬?¨°¤æz«?ìØDN%•Ö?"óâeÀ­?"}H¤—~?uÞÉf,?¶¼Íå¾¾`?•°še'Ç4FGL J1640.3+6850?ï¶oªÕ"©@BgNe¾ ºÀ:ÃfÓ'ºÀ<ō²Û‰ÿ@(j[i@PÒÆÒí?¹Ö°™†¿ %üCÕ9?åƒí€ ¡¶@š¥'Ÿz.?ï¦Eÿ¾'¡¿ãxK é'¿åMåр´¿á¬4Á
!¿ÜÈ+'¢"¿ÝmHmWpAGNbcuNVSS J164014+685231?ïïsÿSiX?]6òBüÖ?4²rõYh–?3ùåþúØà?[ëd›Öõß?Y°+—Wá?ï€ÑZó??
ފâ€?8ˆ×ôځ&?KÒÞðb86?}7d˜Þ¬?}‡òáAÚ?ï&Èç\±?'ú`'‹P†?c‹ £Ä'Ó?R^¤ˆj—?˜µٕ?'ftÎ]?ïÀ?З?eÍÐ4Éh?V>óNvÁ©?Ea«CÛ?z)ÀŒzÀ?e zOD)4FGL J1640.4+3945?ë¾7fÚ»´@D¶¸ºÇÀ8T¢eðõ¡À;r:?–îÄ@àðÎ^È@ ðÀÇÛÌ?§É·n–¶?®ùQ~ç€q@ÂÈ>Ȓ«@úÕOӿܤ–LÝÿ$¿æz8«B8Š¿åÜ7£Û<¿å3"6‹­H¿çþŒ}Qdw¿ï>ÎÝHEAGNFSRQ3FGL J1640.6+3945NRAO 512?ïÒ.sçBŽ?nξäm·ó?Dè`·æÂ??´-Ÿñ?tK¹õaàÂ?mk¨sz¢.?ïŠ~8øO?Š–ü^?Q+I‡'—?cðòöè%?‹;@áÚ?‰b'¥–>?î]'o€ó?—×»þøê?‰	ÌÓ¾4¿?‡¦ÞÛËâ?£ì3¤c¥?"rД9^Ò?ïÌD¶9ËO?i¹Þ¼¹Ñ7?P¼Qs?Ea²ãº]?u®…½—­?h	Êè7Ê)4FGL J1640.9+1143¿ë÷/R¼@AJýTTÀ:%ïpeéÀ<?gÀÙyƒ@;‰³¢x@?Tú-X(?·(xD4b]¿DË*ؓ ü@'drñ9¿é¦Ž¼-ÿØWv¿$·¿èt­Q'Ñ¿ä0œJNì¿çâC5à?ª	CÜ´Ý~AGNbll3FGL J1640.9+1142TXS 1638+118?íØëá"ÌÛ?Ã`릀ß}?x0£_Ð?}?{_+¤a€?¯k-{¹*l?ÃsûÝî'?ïÇ€?"á¡Ïð%V?aÿñ?
o?kÔ­T^8?š?¤î?"
9üFP†?ì f}îù?Ÿ¼='ŒÄ?™TÉÉ®«?‡

_'ç€?¸§™ ¥~?™H6#ŒúÇ?î>o€fã?ŽÌÉIKƒ ?ˆFYmÙ¾-?r¿L{«-t?¦
R¬ƒ";?Š!Ae«ä4FGL J1641.9-0621¿Æ¾Oj0~@9íÇïzÀ9'-åìXƒÀ;©pÑ#s£@
+¢F¨@68ù€Š?·EH´yĽ?ºþð¶`ú—@Wš»ØˆÃ@
ÉÂK"}ü?ïKøQÆ¿Õ}Þ€iG¿âÄßÎ1PÛ¿á߆®Š©¿êb…Ñe¸Á¿ïÿÿ" 5•AGNbll3FGL J1641.8-0619TXS 1639-062?ï®}D\†?}2¡¥?_êôQÝ0c?Y+î
uE&?€|'$­8d?yFTwÎsÿ?ïDª¹ƒŒ?"þ—Oåg?g|mÇ/hN?v)†O›ëŠ?"{¹!}?'Žp!kþ?í¿5fÈâ?šiÚY‰sÜ?"j[šQ?ˆZ~¸SjQ?ªWxš$£?"}E
¿?ì9LògH¤?–‰+ÈÇæ¿? J/?/§Å?ƒoLÏW¤¨?¶€Í-æ÷?'M<p4FGL J1642.3-8108¿ïÿÿô¹È0À6+¢±pPÀ:ŸØvN:öÀ<$iϘ@«FjGœw@âWãì¤?À<'ùn@z¿¬\[p¿?ëXm_)]@ã%Íïâ|?ᄅSK¯¿ãI€2Wk¿íeK´3xÓ¿ä¡ãÀ¿ ;ƒ'¬¿ç·fÔJoAGNbllPKS 1633-810?íbÍÿj?´ä 8kÖ?'¹®KK×?â}•u)•?²˜¶(&¤T?´/'Ÿsý?ï®
hB? UºGso¯?^ä!ÈÔöN?t¹Lƒ<ñä?šÍè"%¨t?žJ\ý g?ëédO¸0?¢-Ø>"á?‰ì.ñçÓÇ?{Dªd±€¿?½wW¥ECù?¡
9"BI"?îe®Z/#?ïѵ#ö2?_bâ¹öÊ?W=ЗÍ+?¨´~]?ŠKÇË©Z4FGL J1642.4+2211¿ï˜Fé@BÝE¶ÃvÀ;rŸ'*_OÀ<£fô*ߨ@!"…]ÓE@°"—©Õ?ÏWŠ€wË?¬"OÓ|ê6?äØ°?ù?G@ž×ÈSkb¿îj.Ýc?ïü_#¦ù¿ëk><{±Q¿Ìm«ÿøž7¿á#ʪ³Q¿Ò^³ŸTC¤AGNbll1RXS J164220.4+221132?ï–5B>·=?"=–ÑÃ?R¼¥&7—3?jy‡Æ†?ˆˋ=ã?6ßLDj?ï?&{Û;?'u%՘Ðú?Wä"v¤Ö?bO‰x>n?–œç==Ne?1OùñŽ5?îZ@È?¨wgÓØ?sݤá›?`x".–?­ªïÜÐ?š7%7¼P?íÒ_Iè?ŸCK—…ê?"Õµ@@

?x¶â¦gÒ?µN¶]¨½×?Ÿ~:F4FGL J1642.9+3948?éا2MHø@Dz'öè)JÀ89m;l½˜À;v†eà/@åëÛóÛ@dŸ¼ÉJ?£<!Þ?¥9w'.?ÿM€k_Ê@;ÿ>¹ú¿Ä©$&%Ä¿àXÔ!Õ½·¿æoP»v­¿åø˞#—	¿æ:%6ñ.¿àpë$¦¨vAGNFSRQ3FGL J1642.9+39503C 345?ïÀþr¶èí?súÿ"çf>?CBQßáþ¯?>‹oA{Tè?}|hIò?s)‡®Ð@?ïwì7.‰?ôjl
)?PŽ¥ùÀ:?]TõÇyÑ?/Þòó?8R$F?îÛë­]?"qZ·øÌ?{Â/0?wx؎:ƒ?£ÂÿD1?'þø®†$O?﭂¥3K«?qÓÞá¼Fa?cÜ`š±†?W^tæ@nÂ?P}gò?oqod]4FGL J1643.0+3223¿í皈×Õi@DC,¥zxÀ:»£?4É5À<#e_Ö)@ð¢S&˜›@üÄÞÁÂ?¿ôPßÁq$¿¡¾ò!M¶?áÓÆÞ@•Æ5ƒðe?ïôŸhËÆ¿éŠÃ=O¿â…yA	Š˜¿Ý|þ®F¿í™z"¿ï÷Ê! áøAGNbllNVSS J164301+322104?ï ¿ÓjDÏ?Ž…Íܧ
?'i]ößËý?wFƒÙåg?'³V—G€O?ˆµ¶õTñD?î´1'°£?œÎÃÍ?i0€?s17:¢2?£+¤Ô4¼?šjÇÅÑIz?íM‹«ØÀí?—y¿ö[?"‰jäêƁ?†²n•D'?°qGçÿFÿ?'—›Z]åñ?ía{ü¯ó?"¸ûÚ«\? 5PRه‹?‰D¼'?©²ïâ'HB?r"ª
˜4FGL J1643.0-7714?ï
‰er`À3æ‰enï¢À:Ϻ×5À<*•Þ#6f@ì¾ÝöÀ¼@$@Q(ç?ìÛÀ°Š¿¥IÞ}â?äxdFÑv?ÿIkjÏ?Ý퍁Þ<¿Õgˆ$|61¿ìÍÛ?¬=`¿Ü³Š;WÄã¿Ð¿'zç&ë¿ïÿüoQÇsAGNbllPKS 1636-77?ïDO×aH?–3¢PR?j)"H|?cs£ÚEÞÚ?"0ìÊÇ¢?•	'ÏÑë?ï+¾ò_y?—Rl4'?WLŸä{?d…‡‡ž#!?™Wµß.ü?–Ü"A+ˆÝ?ì ë3'b?¢ð"ZÇõ?‰´@™è?y"%×?»ÉGžP¯ó?¢Yý¡—)?íšÜ‹^$?™í#Îy™™?w»HVm+?n»0U"7-?µït–>>Ä?˜´/a¸¯4FGL J1643.5-0646¿ÔTÈÔŔŸ@8xoš™tÀ:/<"댫À;ç–{(@ 1"­ú#È@
*áU?À­ŽÙw*.?*äâð?ÃÂ
V)ØA@ÊÑGZÝq¿»z£à…¸¿êßJþ«í¿å.iՆ¯²¿ßµ×<è=¿ä?z™¤¿ØÊ=fAGNbll3FGL J1643.6-0642NVSS J164328-064619?ï·ò×*<?yK`qiÂ?Ejœ3 ìŸ?<ÒÕ‹?€¬Õûb4?xaRô'^?fÛ¯…?ª"p	º'??¼–þN)g?L]ìk'N1?†Z'!­à?Nšª­?î4ËÃ0?•ÂþŽËâ¶?rÏ4ÎД?gë®Z@I?ªYi@ó&?"¦"?8"u?íÊÏëHÌ?''Êã<Ft?_‹lB˜œ??O#+‹Éç ?±+Rô¯<ñ?'ÎA	Ö¶4FGL J1643.7+3317¿‰¼BXB ß@DÔk&¿‡À;œÑ¹ôƒÀ<æݝÕh}@"Yp)]Ç[?ó1°|4.?ݜöZ婽?ïþY!Yl@ÒÞ^ň@%4ºÇ¼˜?ïý*BsÂð¿ï›iGÂ6q?à´®ÈÕÇG?ᇆqž©¿»f͔ré¿å×táSlAGNbcuRX J1643.5+3316?íɜÖˁ?«ßY†w¶?'%‡7's‹?"«aˆo…ã?ªSn÷…Ž(?§86]ÿO?ì:©"ý~\?¼ÄCêahc?¥ÔВì?³[ҋÿ^,?³@KӇ+?­C±V†œ?ëªhó;ž?¥'uO i?"d¹ÃPI?ƒyaixB÷?½Ó‰ö'ü?£ô~ÁªÃ?è1S'a+q?ºj?bg.? ðáØܟ?¦g-Ø}¬k?Êþy€D*y?¹ä×Äû74FGL J1644.2+4546¿ãÒ}은7@DkŠC»À;hEÏ)èÀ<ð1Cnê™@ ºÞ؁â?ýÒ¥Ú¼j?Ȃõ}Åþ|?–g—á*?Ñiè;")@aÒ­âQ?ïï=Û,áà¿ãÃނ׶¿×ñʳ!¿âo‰û–忽àÿ´«˜Ë¿è-Ë_\ªAGNbllB3 1642+458?îܼ†ÞúÒ?š¹®ë ó?[™€Ä;‰?P`´h.½?¡X:Æ
1?šP'#±,>?îùÁ}£?šµéö/ë?Yð0N(P^?iV"z9´I?Ÿ>äÉ-Æ¡?™H7‹ˆo?í(ç
Ï?—¨aáA7æ?v3ô©j³?d5›{Áü?²"_n1ê?–q!ñë©(?î=ù†›­å?Ë^Ïñ"Œ?ibŸ®{S??af¸Þvñ$?ªŠ=›]l‹?ÚφOÔË4FGL J1644.5-4602c?ï…ïç•6¿Éýw¤ý%À8…‹W"<À9ï–
óފ@"#ÆX¿_@Ãûå¿?Êu´¸,?ڄ]<œ›@<Ÿ¡ñVð?øtÊÒ̖¿ïûŸH/Cº?ïåRj0'¿â8Y­ñ?s¿é˜´—Ká¿ïÿý±q&´?ïÿŒýÿʦAGNbcu2MASS J16444975-4559026!? BE/
_'?«Ô;eVU?¢Ø"¥QÐ?«[¬¡¨Ž?íÚ^*åé?´–D蒐?—6ð˜ƒA?œbÜiËO?ٝÓoZóY?ÍëÜ%šH?âweÈÍÂ9?ÍM¼Ì!Ic?¯nVÌ4IŒ?"ž–È*á‰?Ê­‰s>Ü?­øö²‡/?ç]¸6w«°?¯7.ÇB?0?w/§®ÁC?ic¥a¸e>?ÆM¾Ô$?µMKsÅ2?ê>0û™|?µ\Ì~JuO4FGL J1644.8-2154c?îøí²J•z@.}¶™"¡À9ώ—"À;VqÐý³õ@ô¸ßÚñ~@§¸
è´?Ä~eá†BO?©©žŸgäÁ?èyØÔB@ÐUjÀ".?ïþ'ýž%ð¿ÛåB{¥"¿ä'Ö÷ÈùÙ¿æ Üš*¹¿ßr&s!á¿ë†hšMAGNbcu2FGL J1645.7-2148cPMN J1644-21560?ç–ÎÈ?Ãv,+a®?"ß`K"‰?}ÕÅz´1?Ð,á`ÿB?ÃWð0Pw?쫙0çÇ?µÉå' /?ƒ,·Ó'Çj?ˆ£#£[5V?¸=Ÿ"ÞˆÕ?´áÃÈ3·Ž?àÑÞ)k?²x"z…›x?«3±QVã?%,#kK?Úõͳƒ?²"Í­™?ãS&±bþw?°l›Ÿ(ð?•ò~ëZ?€;ÈR¥Ég?×ú'eKMj?°D¥"#¾Ÿ4FGL J1644.9+2620¿ä©Mü.±'@C.}=BÀ:T¨ÎÀÃÀ<NŒÂÂ#@1:¥mbY@ѓpŠ¬—?»ÍÆFö´?´"»;)÷ ?ôØ/ž‹q@
öäñ0Ú=¿Ûdï"¸Ó¿æ}U–4Š¿ê"n§}‡ë¿èç2^wÿð?ïÿٟC&ÆAGNNLSY13FGL J1644.4+2632MG2 J164443+2618?ïõýžÖ?MC擲?Bwœ0Œ]??NªºÁ"?IéXW?B{Å ˜{?ï*ÿE3ã?§(Hº3m?a÷3˜SÌ?w'/¹A?˜a0æqó?¥R zô€Ã?ïÚýÏ?'…'ÇCýÍ?s"¤ßl¹ú?boüñ7?˜Ô2ÌÅs?€ýÔn†#–?ïÆ~;"h?hë(C	Ó?__¯±‡Õ?P)u¿µKu?téuÔVq?dRÝdʳ4FGL J1645.6+6329?ïhýتÉ@Bü½º
RiÀ9á07Ö0#À<hœo6ï€@T—Äw#@
‰ÎÒa?´¯[ø¤A?ÆãÛÅ~@<œÆtÃ÷@T)`vP¿Ó‹¾úýÚ¿àö4êK¿æ,%!øxL¿ë´×Á¯b¿çj¯Áy1š¿ïà18‡0AGNfsrq3FGL J1645.9+6336TXS 1645+635?ïÚ¤\¤¤ß?p²
Ɲú?Yæ@ÀÙ£A?W·{"Öþ?hh'úîO'?hæõE졶?"Rï?Ž'.y¾6¸?Iè&U(+?VªµM»ç2?Š5»õ˜ºî?2²r*®?îS¹¢›=—?•Rщ–ˁ?îåb‡ßi?†V˜ºyÔ?¢Ló%6¹?Žï̌>wß?ïÕµû!q?^ua†®
€?[}ÿÎ?JýAtïŸÊ?lºxž?X¥[-´ý…4FGL J1646.0-0942¿à÷´ûß	@6Lp¸Ï¿ÆÀ:¬~T–ZÀ<®Ò@!2ëÇ@¦¶~¡Ç?ÀÝYâÊe¿©—ÿ™jË?êᡥו~@":îéW¿´Îž31ZÁ¿ìÔ)þ+>¿Ïؓ)'ög¿çÀXëS '¿©à¡•ø‹¿åý
a½_GAGNbcu1RXS J164602.3-094113?ê"Šïžd?º¾AÉû?'~‹QÕ?…Ü»\œ³½?ÅS"ì3?º;ßÁþ?í
ò­~?¸5ú5€?zQø¬?ŠËDž¿UQ?±ò~¨âP?·tiw¬OØ?ëgjŽ"¦?¤-=ü×?"H9<}Ÿ
?"=YЫË?Á…[.69‡?¢+Ñ%'?äm"ÞV™è?²Åv"_?xÚõ%`®\?u
(ãH¼?ÖÁjn½Iu?²î‹NÊ%4FGL J1646.6+7422?ïçƒ'¿á@A$'žùTëÀ;^#QA;À<ñÄ>ˆÑË@ï·=ïNØ@=â@ÒX'?Îð颜Ž?Èùª¦\J¯?÷ôt{Òß6@˜5ÁWú?ï°û€>~Á?Ù=B äfœ¿åoïaLK2¿âhˆ•â¿ä²¥¤i×4¿áþ·á-VûAGNbcu7C 1647+7424?ï‰6)EŠ?€ÏP'•â&?aTë@)$4?YIXb·¶?‰]:ޓ¯?~pJ\ ?ï…AÅÖæ?‰•—ÍYì?P=Ov?\ñ˜Ïg>,?Œ¨Ë d?‡Žtþ?î
UBÆD?'Ý|#‡¯%?'F¬(-ø?x	0£Vér?ª™ɐ@³?†Ó0(3?ïg'<W½?wR­³"ÿ?tô¾"Õ?c1®ÏK0?Œ2¶‹óv?slíe4FGL J1646.7-1330?ޕpo~½ö@3õZž²OÀ:ΐTvyÚÀ<)VlGQ@"m@JGø?þ¼I	^N?ƂcÇûÁ¿—ú¹š?Ð$ñüÝ
Ý@/¦(s<?ïüÇ0«™v¿éó5ò*T¿ëOŸ_¬8?'3CaK¿âFîœ*m'?¯¾
þV˜ÏAGNbcu3FGL J1646.9-1332TXS 1644-133?íÕÜÒ3/Ý?¨Ç™²¹øß?Q'œ:+íÜ?RwÌՉ¼¶?±
Òý}Ñc?¨Ÿ°¯e‹×?î´,°,W?¬"ŠgÈ	?ddFgÏ)?}%üÉ86?£vûN€Gù?«^õýå?쪝þƒÇi?ŸË2wA?uƒÜ‡Wæ®?gkd¥Tø?¹RÒClFO?ž¹ÓOS?ëcJïL
-?§Éíß2¹`?v§I§W?p®Ö\T#l?Á½› †æ?§È­yæyð4FGL J1647.0+6040¿ê‰+"½È´@CAÚßµÝÀ;s €©ÌÀ<Äæ©å@àfgh@±ì¹ÒE?ËD௭­¿vÓÿŠÓòË?¬1¦|g?æ@5=†Å¿ïÜD¿L±‰?ïRuÚ¿èsûÿwD¿Û+κã–=¿äèÏÍ2MZ¿ç‡Jw—AGNbcuNVSS J164641+603930?ïÇg¬ÀEÖ?t8þ‰"É?MkÃæ³çP?H‹ÃÔÀ?xž±#˜*?r؝8F<Û?ï±éuÙ%Æ?'UÆHR'|?7@°œOd?EڃÔ9aŸ?'˝Ô[?È'@CtÆ?îOõ¼ÍEå?8ß'?ylú¡q2"?pè"ˆJvU?§ÓÞý{g?‹ý}KdGd?ï¢.x‰³?m±%cÙF!?\BQs?J"…¯n.+?ƒñÙ?õHÆ?lw]Û34FGL J1647.1+6149¿åG EDØ¢@Cvÿ:Þ"À;AºrW5qÀ<éegÊ@:¹•?úƒŠéÓmÑ?Ôª;þ2öL?ÔzJ´Y8€?ûϨ´¿Í@G¢ŠY
?ïý#I±$¿íÙÁY|¿Ëì쥿ÖÍ.œ=¹¿ëuäޑpU¿Ò|¾aÏþ°AGNbllRX J1647.3+6153?ìhÝQ_އ?´"©ãŠV>?' ¡‡"'½?ƒ'H2-É?ºuD¹—?³ˆŒ¤ûC?îÒώŽS~?›[Öf_®9?j{€;?v(ðÃ!‡?¡*.j ?˜ÏUˆµ:³?ëë™ýr?¡x»Žßœ?žÜ°	—:Õ?ËNs"?¸ì	<^?œ}º÷o:?îGEçF?Š)ç."Ñ?u‰âu{ϗ?flkŒÊb$?¨Úe@,2?ˆÁȲj4FGL J1647.4-6438¿ÁÅ,‹_€TÀ(íêî ¬À9€éNã'âÀ<fåè&Å@4$ÕwkF@
¿@óW?±.q,"?§(¹vÙ¦?õA¼bò@ˆWƒŸ‡D?ïñ?Ù}¿à"P&‰Å¿å"ÈL4‹ù¿ãJ=Á+®Ú¿éˆŽ^Òô.¿§™(¬AGNbcu3FGL J1647.1-6438PMN J1647-6437?ï®ôÅ?uñcÐ㛕?Wršå8Z¶?K½Ó£Þf?fòkÃ?tßúÌY?崙/š;T?ÍéùÒ?Eý'¦?TC?d`jÈÐÄS?"ºÛï
5¡?Š²°››G?ï³|œ$Å?Ø!üÜ*¹?p9mɅYm?b7Ž°y2Þ?›4ú?€3̃Ç/?ïlšëx?€-"a–Í?}XôïƒÈx?bëûËêò?—</'¡žÎ?|Ë°ôñÚ¼4FGL J1647.5+2911?îdÓð
G4@C='Ýãu†À:É@š$À<gzbœ­@Ë["l@{k{y"?½†ý )Uº¿¥2!BùWx?è:±âe»F@öü¢R{¿ÔÖß?–¿é£(Ž"ƒ¿àSþO%Ø¿çOÞk…µ¿Ò34	òÈ	¿â^"3N&AGNbllB2 1645+29?ï"{Ú?ƒ»}ç§å?`^óöÖý¦?Wv»›¾¡Á?Šä¤<S¼Ñ?'¦s?ïœ=Kq$õ?…&wXÒá?<–Œ¦Å˜U?MÞóL{¯?ˆø¾€•x?"u4L?îb­×vN?Žvê9u?vø?(܃?j}–ó+W?¦ö£Â?Šÿ]I(ӓ?ï"jèZX§?tŠØ $¿D?YòÁ'?OÐyLÊË.?‹³''ID!?t$NZK4FGL J1647.5+4950?Ô^A{—ÈV@D	õ­–¦ À8ú'ûnjÀ<GùsôÄc@Ô)«|ñ@î¸D‹Ñ?¢²o~hß?Ÿ}ÀzNŒ?ôQ.ül͉@3L´äx»¿¸þö?·Ðç¿âíæÝð
¿¿æñਠñ¿äìö}Ë1í¿ã¼¡Ü^:H¿äÚ;JXêAGNbll3FGL J1647.4+4950SBS 1646+499?ï gí_Uå?­5C†'ÂA?NP†¬…à?|Õ1"'C?†ü=j.n?©·
aÄ·´?ïÖ‹	¯º?ŒtX9Jì4?LËnOpfÇ?]ö>šq4n?½¦X
Ý?‹Köµáˆ?ï;_ŸšI?GˆÓa®†?g30ÁOU?Rþüm>Ì?•¢e¦£ìç?€Œxqo?ïêƒÛÁ6M?TäØÙõ…–?RäXQ?‹?F$8\#%X?XC%B)ü?JõµÖÓò™4FGL J1648.0+2221¿å8ñ¬2Öõ@BD±ëÕÀ:!Øb,EÀ<MˆGa¾a@¾úWI'ñ@7~0‡‡?ÁžsˆØ›?Ë$ƒB@† Ä0F@b=Í@:?˨c`øh\¿ãR@>´q¿é†k>'aí¿ç<ÛR¡"¿ïÿô¬å¦¸?ïÌ®.|NAGNbcuMG2 J164800+2224?ïƒÜÄiþ8?•éÑMË?ƒQÊ&ZGœ?"€"pd?wn	~LTB?yØÑg"æ?îi…¾ý­?§DºHô0=?|wlD&?ˆ T7æ(o?¥Ø¶‡¤Œ>?¤.ÁCcˆÌ?î…ði?•9má¨?"'3Ú̍?†²Ü"4¾ã?¤v‡r'?Ð'Cˆ7?ïHóñ±?ƒËò`Õ?ƒf²*¥ŠÇ?r
?V0VA?"ˆlwû?}Û.U	&Î4FGL J1648.2+4232¿Ú`áÐÁ	@DË)^žÀ9¸xq*å‡À<wÜygË@öO+â1
@0‹¹F?±àÀõ~å?´
šGiv?ý œ˜Q›@ýuOÐ?ïÿÿ>¹ú¿àW¤ª²¿æg9ª€¿å9‡`1&¿è¾uñô¤'¿ïáãµFžJAGNbcu3FGL J1648.0+4230NVSS J164831+423322?ïÛ—èwß?qòOm_?;‹ÄÑÖH?5@ÔOÍu?pÄ÷¾²£Y?qS;"¤¿?ï F,A?…ˆð¼	¬?F<¥»=±ž?V£ZY1\?†›d;àe?"k_Zq£?ï§'¸Í?ƒcxí?pá\G<%]?fi:YŽ0š?™R¶ÌYÝ
?ƒ«H:P?ï䀟ó?TˆÞ4??U^	Tì?Bq`a;^?`ÐùšNý¡?P–lÍXùe4FGL J1649.4+5235?²ø,äôèž@Cĵ¢
ÜbÀ9*ÃÁ‹P+À<<ôE·š6@+Xäʑ@J¾A?¦?·>ßÓ?ª|·õ@EøÒåÂ@à?pXX¿Ü
²ûjo¿ßŸÀdµ¿âra ä½¿ÝN	îû̿䆃—¿¥¿åõ'ž}¯AGNbll3FGL J1649.4+523887GB 164812.2+524023?ïìµÑïR?\Z)a›=?/n÷ãHî?,î¨0áÕ?aS?~Ü!D?Y‰ôjÁæ¦?ïŸú3¦è?ƒ<¦tC"n?Eê›`h€?Xú‹KæJ°?†°Š	`?t?Ô¢T¥B[?ïK3­«ø?y•ŒáàßÊ?fµà4A?U†¢×®&?"Øs¨$øÝ?w­ÎG<?ïâ?kæš^?U&SccY¿?LG0¦äð?9nØ?$t?f¿'M;è•?RpƒC±Ú4FGL J1649.6+0411¿ïõêØj@<åý2Æ&À:!$^"ÖÀ<	"&¸Ñ@J°7•Ãv@ürâu«~?ü}õ#X?ÆžÙtzü?þf"¿?E@Ý\"è¿ïÿÿ)@k*?ïÿúÁҝǿé¥Ñ¶@™M¿âO¬{­¿ïÿþó…õ?ïó˧nnAGNbcu3FGL J1650.0+0356PKS 1646+042?ïÉ5OµÀ¦?'aÏq?l¯f|T
?t£GG']?jJIÃl?x¯B…>Ÿ±?"´$™?Ž6uë ¯À?UŠo¼,¡¥?gjxÕ)à?‹­ŒÛqE??Š«Ò0A÷U?ìçº5gó? Mõ¶'ËÕ?˜¸¶ÚÖ?‹ŒÛšÓ¥?²ÀÏI­?œ$mè£ýñ?h¶bq?vk )›VZ?bÒ[g?S6Fº'C?ƒ+"QeŒ­?tçýYô£4FGL J1650.3-5045¿ïÿÕfŠ‰ÂÀÈ þÀ7ã',"³À;ýº@¾
/=…G@žÞ|øy#?¡ƒfÁþB?§bܙË@ô6%UúÞ@aŽQ?ïûûß	s¿äT^¦ÿ^¿åŒ|Dôü—¿ä÷'ê)Õ¿ä˜æ€Òù7¿å÷>àæ_EAGNbll3FGL J1650.2-5044PMN J1650-5044?îèŽaž~à?£ÔtӘL?Pí'52?Vxâ9OËù? ö'«ˆm?¢Æâ,ç?ìûÛá¤?¸Ý>ëh'§??*w1Û/,?Ue5R[:½?¸üùƳ?¸Á¬ªk1†?êÑÁQœ?©*Øóö?"³½Ã[w?Šº-­¸?Â#nƒb!?¦^y\0Ù¯?ï!Ü:ùÔ?ˆðáûHç>?cèmðˆ?VVgÆËl:?™zjâÂ?‡ù»a'aé4FGL J1650.7+0831?·ùtRe½@>¥¸fä:¨À9²rùòŸÅÀ<<(¥:¸@Ñ
NG6@Øró<£?¼¸«­˜T?Ãy§¶½ÁÂ@°~ZxòZ@SaÅ¿ÀŽ|2iµ¿æï<™
' ¿äE`ýpه¿ê®HÌ]ç¿ì1  œWº¿ïÿÇ*Ì\eAGNfsrq3FGL J1650.8+0830MG1 J165034+0824?ïuÝhUu?‡rU=7i:?wÁð'ðŸÜ?p"ï?ç€o?†§­–2RÎ?ƒ¸?ÂÎ?ïc'TÁð?Ž'U:íN?a¶z/?qq&Ñ	J?'Urǘ€?‰™‹‹¦14?î˨dpo½?ŠµØ]"?€ê'0ú…P?x£ê${<?žßÙtÅæ?"Ë·©æ?îÔÙ8™j‡?ƒóu0Ó?…$Œz›ÝÅ?p²Ÿ+'$?šÒ'¯"À?€\}9«Ó«4FGL J1650.9+0429¿ë€š«â@<À%á;ÛÀ;Zœ-ȐÀ<r¹¸óÑô@!a‰óß5Z?ü«+­,ôU?ЮúS?µJ;"ý¾?æ5™e—4@Ð}
œË¨?ïÝÅB"пîJn×N0¿Ö4œŸˆpý¿âBá[Ð
o¿"*å(Z´y¿ç"Ғßk5AGNbcu1RXS J165053.5+043009?í±½Û­?°³B!©‹?cÓ H?Zï:àƒƒ?¶ŸÕâ"?°ysˆ?îwŸ'.?­½¨6åd{?vDoÉÔúÙ?‡…Å+Šh?¬ªŒÒíÂ?«CÓri&?ìîÆ™Ð?œj¿›ŒãÓ?x~³§î?f÷ŽÞ"?·䙄OË?›W'ánâ?éiÅ<LžÂ?ªÊ¯¥L
H?k=ïlná?f3èÐp-)?ÉìzÓ=?ªãI¶b«04FGL J1651.6+7219¿êl¾vÀ3@AZ*o?RüÀ:u¤åýö;À<¨ÃФÉ@ €ç®z|H?ýùiÈñuú?µÕáswñÔ?sñ‡l?Á«Ü<Vr}@bô6H;ƒ?ïӟ县Õ@Q~Í»_¿â#îâvWJ¿á{ý§`+º¿Ø"ÿ^ow¿¼âÊ [PoAGNbll3FGL J1651.6+7219RX J1651.6+7218?ï[œÚ,Äm?Ÿ‡|/N†¶?\°Sïw?bõ>—£Š²?'Á_ˆè'&?}éo8.W?'ŽÎî?†ˆÑ¾ýî?G2þ´ñÕ?Sû'Ùüg¦?º|`õ†?…¹‡ë´?î8'nÑø¬?¹ÄÂÃh?tžÑ9Tz+?e[#4'þ%?©ßÍ;µæ
?m
y÷v;?îÉF"B?…£ùìÔöx?wãÊÅëáv?ceÆsa£? o%i?À?…µò'Ÿ4FGL J1652.7+4024¿X|Ïq]^'@Cb¯È°À:™":ÚÇaÀ<q.~˜ŒS@ Úàl'Ο?ýC$\֚¬?ÆuÌ4÷X'?´o"3,'?ñÙ«Ø`@ªÅ
¶'N?ê&둳ò
¿ãþÀZN¿Ï¥_ö_Ã4¿àXŠp0ꄿÜ®½î¸¿Þ˜âºtÛAGNbllRX J1652.7+4023?î†èÞ±?–ù'¬"Ñ?TdiÕõfï?C:R—å:?¦úÞ#e<Ù?–ÀqÄIç™?ï_¶þ3?‹•Á
YóÙ?P.ì}¹B3?Vïñ'™Ïˆ?"!D¥b?Šgf=ìF?î!!H8äY?'¾£0X¸Ó?när"Âß?ZßdàE'?¬]5H~K?ç¼óøÅØ?íƒ;ÝÀ?'Bâ9ó:?w9q	A?cùO¥Š·ê?²rp;ë?'_?²¼(4FGL J1653.8+3945?ç)Nû22@CmZ¯xþïÀ6Ę¹ŸÉ_À:½¿_ü¿Ú@7o¡Îqh?û‰¨U?†?‰i<¯ˆÄ4?"hKeP‰'@
gý?[`@0''àCÍ?Ú+Ú佄Z¿ÕÇ+£ù[¿Ü2Ÿæ¿g¿ÖPñ_(Y¿Þ"ÊÕ{Ç÷¿ÏU)¶³AGNBLL3FGL J1653.9+3945Mkn 501?ï¨E]SxÅ?€¡åýÈ?Ô?<"_›5
î?6|A7ë;?…
•®H&\?€g‹sGÖI?ïSG™Ê"?—†ñÜ1$x?T†'Ç?-?eé۳٘?"V"s
G½?–ÃÅèÆR¢?ì=â̝û?¨±ûøٍ?"ÌÓWõ	?'G(9'h?»wO0†>?§dŠ>×0?ïà{X-L[?c®ó
Iò?#žÖ[æŠì?!áƒH³V?nJºlõ<D?cj4‡×f4FGL J1654.0-3509¿ïêÛÉ@˜W€ðUhÀ9ª6CˆìÀ;'ã}zV@)Bnº@¾aÏþ°?½n'¥áP'?ªŸÀÊØM?ïºÿ?8$@Øד¥8ß?ïÿ®©Ì¿äÿà iA¿ãpWìPÓ¿à¬ÿ'¿çõò•´1Ë¿Ô©ãßVAGNbcuNVSS J165404-351301?ß,áäâC'?ĸ®ož•v?"¾Ù­"ÿÊ?|1:þšŠ?à"¦ØÊm?ĤzØ`à?ÜҀ;C?ŔׇpéÑ?•b#ÀGs?™,ل¬Ç?áN3®Öà"?ÅãöaW?à'?û>L?µ§·ÙÄ#?¥Ó4€ü²"?ŠøA%<V?ÜAŒïéí?´¬¢¿ÿhø?â;4ðÀ§?¨±-•Ëá©?¢ëYy…v?"v–ó^Ò?Ù,|fíÏó?¨Hý¢áo4FGL J1656.0+2047¿îü œz@A$äâmHÀ:!ãû½{ À<RNöÞ@-â´?¸'@ŋûKeY?Á'ï@À£?ɹÀ€Ž/Ù@ꇅšß@8q¼Æ¿äDFŽ¾¿á[©t0¿æ<ït—'¿çlãË¿ìK`†R"ø¿ïø¸®1×AGNbcu3FGL J1656.0+2044MG2 J165546+2043?îâˆà4'­?›dÞ@Š?‡g"ðk±?n-tóæv?—ûa/wt–?—B…ª£"[?ïm¡´â/—?'ˆÌfUý?V4_˜ÏjÓ?càfΙ4?èƒj-c?‹šŸö‰
1?îúŠú?˜
§&8:C?'QëXÅ?†KBôŒ?¥]*ªücÌ?g!‰V¤?ï	}¹:¾?ÝáȎ)(?|@½™:?cÒJx_d—?—À––F&?Ñ?FI¹4FGL J1656.3-3301?Õ@ù	k¹Œ@hH'ÓÀ8ç
ÜÒÔNÀ;)yÙ	ò@ÆGåœÒ^@Ršäó4@?º­j˜?Ót¯'@T+
oÆ@"4A{†¿Ïñ@õh¢¿ä^2.o¿ê¹Ë"}®W¿éY<a°@¿í-F¿×ñÄ¿ïÿηˆ—êAGNfsrq3FGL J1656.2-33032MASS J16561677-3302127?îØ~¦šIw?£«n˜:é?™Pk=s7½?—ÓD¹eg`?‡?އ2m?Ÿ­!n=Æ?êš æ–?Æ*}#Àj?žiÒE¼û{?°Ý<¬ky­?ÁÊ·5@Æ<?Ãe'9ÄÁ?äÿ+é	ë?±ß—\÷´ˆ?Á•8r0D?¦©ŸT*ô]?ÊnzT¨?­¶!ÓÒé?è0;…íœù?¯ã£´n[
?±¶`‹¶«?œ†Z' Ú?Æcᢽ0Æ?¬ýꄏD½4FGL J1656.9-2010?ÞRoêÎb@,5inX£À9j›‰]â3À;âxˆ§ÙÎ@ z—éJ?ýT¼ÕÞÄF?´³£(2ú?¸öª蟑@í^µ˜@J4Sï–P?‡µöØ %á?ïîÛJ>´¿á2"¢¶‡¿ÝœŠ$[©õ¿ÚºØƒA&¿àäõ¦n"AGNbll3FGL J1656.8-2010NVSS J165655-201056?ï˜<|Ý@?ÐCœîI?^¤­ðâ%?UŸðCÏw?†K@tóÐ?€Å»á6í?ïç#[Î?¢µ³ï ?kÇ4¯G1Ü?|$.cãmf?›&¼…« ? ¬pi'Ñ^?îå	«ð?Uÿä60?uS£ÇÓ­z?l¡?Ç¿_?¤w:öºËo?ŽWt•)?ìC¥lÜ?—5Â~ÓP5?ƒX̄žä?…ùêœé®¸?¸…¡~Ñb?"‰M‹»óm4FGL J1657.0+6010¿¤7êeڒm@B´iaÃiwÀ:~oPóÇÀ<¥ôõ
¸@™'Ǿ,@cg]Ý*é?¼¥nS"Œ?¢ôšàÛ;i?äXy¾²Ø°@
	ú
å¿á†*Qb¿âO¾Ÿ !¿æïŽÎd|¿â°ô>«·S¿é¬¶ApØ¿ïð‰À]¨¨AGNfsrq3FGL J1656.9+6008RGB J1656+602?ïÉ—ìçm?sÁ2£°e?Z©Éѹ?O®P°.ý?tï	—Í?r%ȯæt?ï¢î£?]§?"'`ýB×Y?E¼±^)t?W2°Œ6Í.?…èŒ?£x?'¡V¥—ìN?ï=JIß«ý?~a®äÀd?kQ¶Pž)¾?^èYË¥Ê?"ìùö»?zÁKX:~?ï­¦—ÌÇ»?hKuÁS¿?iìy–ý†g?Q½íè?>´?|6wN_ö?dªˆŒG;4FGL J1657.7-6120¿¼š—¬•°èÀ&¶"áÉ´À:ˆ™'6À;èZ§ìB´@>tà&ƾ@Nõ>M?ƛoG5ž?rŽÛ"T¥
?¢bÕã ÷@`Ü&$?Þ©'`ìÿȿꯍâ+XÉ¿çù¥=;ʱ¿Ù^–C"êf¿ë2ˆä?°¿€m»qAAGNbcuPMN J1657-6121?äÍ«½?Çm¤…!¢?'U¸3?†
Kîœú3?ÕÎÔâ{%K?Ç:³ÿ$Mä?ê—ÀÍãê?Â~>aÁpÙ?c!!øm²?p߀d	Ѭ?ÇMv"Ž£?Âbœ·ŠŠ?罧³æ:?¯6öPgé? 7F?ˆs³á?Ìû™kaÚC?¬ŽÔM€9%?ë_N¡É6?œú÷ž*ã?{C×o¡³Ã?eßþH%	œ?Á¨¦À7͈?œ†¬ì`Žo4FGL J1657.7+4808?àI¨Sîh@C=½øôsÀ8'BhZ\mÀ;ü¯0ړ_@mE÷0"³@xÅÿS1Ö?¡"ßíª­?¼"N^‡Êº@	0¾
í)@q܂!ƒ?ßê
 AÿT¿âɱgì¿åù»þHoÛ¿ç	õíW†Ð¿è"9-H8¿ë3Ÿ¿£n…AGNfsrq3FGL J1657.7+48074C +48.41?Çáâ?"udš3$Þ?eT¼jOQé?r&d´ð?‰)«ss²´?
vÙÛH¾?À•?œ>.""@?cOiö³6~?pÃÚÞæȀ?šÄ'1†"?›¿Hˆõ|?ï—Kðó?'±¤4ey?v‡ ô¥Ç?r›À¹Ú¨À?˜œÙXoµ?N¨"Cãµ?ïÇaÉto°?f€£t²ÅP?ikO՘1¤?Yåê'?o2æµø7?\ó@"4FGL J1658.4+6150¿ìó]ýƒ›@Buø"»ì«À;
ºª‹YeÀ<ÖFô@>#âÞ1#@ _¼(9Û?Çõ°[R;?¬`j_*™?á6É™"{@([DŸAN?ïaÜ>ñ§¿ç_d¥Ï2¿áȼœÓཿÔ|y"UÀQ¿ëþáòο¿ïì=ÆþAGNbll3FGL J1658.3+6149NVSS J165808+615001?î'…x]M°?¥rÛ®\dB?tɞámoß?t[€ J—L?ªîtývò?¤7°Jýñž?ïó—ÁM?"¦'Ë÷݃?` Ȇó?gñüöù_?šøý‰Ś?'E*N¸Ÿ?ía'ʒÁé?˜áy~ð<?ŠÝŠå¨*?>woŠ?±›[-;®?•Týù/­«?î»x+$ì?Œs¢In?'kafò?xUWah¿?¥®Â̌ý½?ˆh yt	[4FGL J1659.0+2627¿îct-K¡@AªÅO±À:±räùê<À<Q
¯ëëv@7;Îßw@'¤/?ÎÖç,õW?Ò(ŠBŽšã?úð"!'÷¿@ßëR?è0ál—¿èt9rèU¿èB¤À>I¿ìCŒFÊ¿¬¿æÑü·v#s?¹`4žWµAGNfsrq3FGL J1659.4+26314C +26.51?íé"bœ4?¤ô!ÃÙT?‡¯ è©‹?…[uXðvA?«'!œc?£w©Ñl¨?íY"œeÑJ?±Ùc¦@?"=qÛÅÈ??žyIxåàg?°gŽ¥à§?¨t¼†Z‰?ìaW–›ÔN?oˆxl}™?™²J#Ä0?‡Ð‹4î?¶²V¸˜l€?˜;úP€`?ìç{Ãã+?˜
Ä8j°
?'"°W	y«?~k>qlžâ?´;¤ˆ??•ÈyA漣4FGL J1659.7-3131?ís/¨¢@Òø_øŽÀ9@Bæ.žÀ;'ëƒq9(@5ïù>@ðú#G,å?³ÊL¿Ì3J?µö<Ý«í.@=Õ%`â™@¤÷;
m?ë\ûÿr©¿ãt›Gï'ڿ收:º2¿Þo•¤—y"¿åeüH»Zµ¿ëÓŒÚnvAGNbcu3FGL J1659.7-3132NVSS J165949-313047?¡h˜Œ?™[ylض4?RaÓ¾"?I¶[Ô."ú?¤erà‡Ù_?™	뮲ù?êçÛY&µ?À\'b"ïB?o•ú´H‡?0"ÈpFÝ?Ãâ>/zZÚ?À*εÏS?ìÒUµk¥?Ÿ{~¼¢X?"ÔXºh¡?u`"ϑ~ä?¶ìwÌ¥UÃ?œé3vÎDN?ëà+­?—:I·Vä^?šëÌ_h™
?€dÕlE?ºD0fÍb?•\ÁAgT*4FGL J1700.0+6830?âC!3Æï@Aš¸¾øγÀ89FÍCëÀ;ׅJW<'@Â]ûu­@:>xá"?›Zm^Ó!?ºŽTììQø@ÙùŸ"®ž@TÖ}АQ¿Ú Ä܏û¿á1ìv¶?ÿåÚò)}¨¿æóe½Éû¿êÎ[–x¿é\°9ïAGNfsrq3FGL J1700.1+6829TXS 1700+685?ï8\kğ2?–&	QÆÚ?yb6š76?…Ôb1©ì'?'›Ï9ŋÝ?'ÅÙ;ú±"?ïoã|ó;?œÍô
tµ?fõXX±^ú?vzh»kÌÉ?™sX…KlÑ?›
.|'?îϽíÅK?•iH0Í)?ƒ},ƺ­?~£­P&«ò?œIÇtãùW?'`0íȹ²?ïâU6§?[wÜo}?UàÊ#É?H'l«h¨º?cXºdlÕþ?UZ$òaRµ4FGL J1701.0+6613¿ë,©ÿ˜Q@AÙR*o?SÀ9ì¸c­OÀ<y7ýO1@ë‡('çP@ÑBªŸ{?µ£*€ËÜ&?¨o¡"2
?í'Q;[÷@J¨¡tYn?·ä£Ù
¢Ö¿æêµ`I–Í¿è"œFó˜¿êƒCÿEÆ¿êí«i¥¶¿ïþ;âÐAGNbcu7C 1700+6616?ïßÒ¼7_?e€Üèc•?QÖøù}—ù?F~ÁO"b°?gB}Ç	Ôµ?b›'ÙÁ°?ï^óÚ¨:?'ìƒë~—?`P3éE¸?p5ã,CŠ?'=w~-Ð?¿ögÜ
)?ïËý
"ô?…;µÁw¨9?qPXréã³?fôãȹ?˜'jA¡(Ž?'Ù·æäŸ
?ïnò"r?yeuaöEþ?ƒ+@6@¤œ?qvS¼Ì?7%âÛ6?n2"ª4FGL J1701.3+3956?؀vœXTš@B¹Æ\pC_À:1!
;ÃÀ<Žgú»¡@ø˜¾ñî@2<ã¶^?ÆMO~˜a`?ʇò<ÈÞ+@£¼ÅîŒ:@GhÓ©	ú¿êZ…¢kÐ3¿Á‰¥…¶
¿áúâ‰Ít¿å–¸w«¿è×ãD8>¿ïú":½k0AGNbllB3 1659+399?íϦ¡üf?¢ñ˜@aŠ²?Ž#IÏ/p?ˆ§Aúóa?«

ÅÒw? ääkVê?ïKE‹‹&˜?…ƒ˜|à«?`܎œ"ÀÞ?lÐå"sß?"{¼»"½?5ßÓÆrÝ?íµK`HÁñ?–‹ËLY?'ŽDÊÓ$?…ýW%ý~U?«d'òw^? äUûÛ?ä®ä?"Ì ö,š?Œ¹(4]PO?qœ"°"¶ñ?ž°Oc{7?'P0å*4FGL J1701.7-5621?ï|
þ¬À!Œû¼¾bÀ:f/Ш# À;—Œ™¦@4›Jž´·@ >ê šª?È Br–K? "…`Q¤b?ܬ®^͕Ë@Zª=€¿?è›×âTžh?ïÙ_æÌR¿éùJn¹?¿è¸æ0K!g¿Î°Ý˜wÄ¿çë$ p¸ÐAGNbcuMRC 1657-562?×îgû}µÂ?Ç(FšóFG?—'¥5ze=?¨Ì	ªÚ®›?ãL>ؕQõ?Ǔ?îÚԂ?ãë(ü˜?ÊJ܊äs…?v2pÿô%N?†Ž|î•:d?×Ñ®6=?Ê,<oE]?ÛÖl7¸Ô?¯àM滹?©xŠn?&"YŽ»œ?àތ(ó¼µ?®qeº9}/?æÄ/¶íQ?±nÉ '3o?'U§³£?‰‡	Iil?ÑROG´©?°ñ#ó!Î4FGL J1702.2+2642¿åD
ŠúfÛ@A\‹ÁiÂ;À:"E>ÎqèÀ<ƒ:"ÀÅ@%|nWÌ@®M]€ä—?Àóîº2kb?¬±<Úý?íS?ˆÖÿ@	d\1"1}¿ïû>¤€?ïÿbì^bŒ¿ãrí]f¤¿áÌ@µÒµ¿ãˆpîèV¿ãÇ(žáŒAGNbllMG2 J170210+2643?ïäý‰¸Â'?•/k™Ó?6ù+MEô.?0F6ëC±ú?h#Pݔ°?•1•…k¤¥?塚0z×?")èWzöÕ?C'dñ
þ?S¿þºëÓ ?"¢â$Ш¤?'Öoj¯?ï>èÓ&x6?wˆ²ìPØ·?dh TxS}?P«W6ßy?••Ñ¡î²?u6Sè?ï^ ä´·?tȤ÷Ô_?põÑh=ð?Z'áßå?üÞD3ÚU?s€39n)4FGL J1702.6+3114¿ïü—kÓ@Aߓ‰µ À:R2#h»À<vòS4Z@ P‡[SÇ?üoøØ?¾Þsþªjw?³%ÏG{j?öh†>Þ@\'t/'?ïÿþBe«+¿ã¢UË
¯ì¿ÝþÄ+=›l¿Í¯u£ñp¿ÝÒõ:ªú¿âÁ<£AGNbll3FGL J1702.6+3116RX J1702.6+3115?ïbÝÏÈyU?"
÷;
-?O¼¡'5?I«鹋?'¦`ú\[¶?"˜îW$RÃ?ïfƒb[B?ŠŠÉ™?U;c[챍?`ùá¶oa,?'Ûæõ̐?ˆ#-;Øþä?íªÁusY¹?•LÓ]2ºy?y*V&7I•?f¸ô±›àÑ?±Nò½ž?"ñ½›†_0?íL]\»,i?j7X~?…ÿZµnC9?p(Þð¹T?²Ý)ÃxÔU?ŽØ9l6n4FGL J1703.6-6213?Ǥnß±«ßÀ(â­ÄÉÉÀ8=֌i/oÀ;aª‡'§@G–¡—"Ý@áª$+Xs?¢þ\緊?ÃXeœ¼ä¢@Ê&½+.@Â*f…ðð?ïÿ«çy÷=¿áˆ¶‡¿åñ°F"HϿ婼'ì&.¿ë51ÛD^Õ¿ïÿø="ßEAGNfsrq3FGL J1703.6-6211MRC 1659-621?ïžJ©û3?p¸e›?w;YA
÷?wÅ‹!åé?yŸòÑÁXG?qóV-¸~Y?îÃ~9/R,?ªÄËÞÏæ1?TQñg¨?'T¡YV?ŸÍ#ř`Ž?§Â]ðï?ìIþKœWi?§¹Þ´Fþð?±H²³BoÓ?¢cüë8¯?¨Îµßµ©Ê?—£Š©6?í)9~°¹? i'™°·Õ?™¿¢—±BX?‰¦ñ[ b?°FKj)¤?š³¶z=ƒF4FGL J1704.1+7647¿á_ËWµQ9@@1éÍ³}À9@UÁF‡À<M¼¢³Ï@¬ÙIÝė@S°ÄXŠ?§ŒàŸ©?‡–!jŠ?Üî~Î<9@­ÿ±%§Y¿ÔȨZ§–\¿ä_ÕÑXM¿èO/]e¶¾¿ã_lÂK¥¿éï81Ÿµ=¿ïW–Š •AGNbcu3FGL J1704.0+7646NVSS J170357+764611?ïäe
¸nÞ?d=¥]'éR?P]ÿ¨þ?[þy¯§û?clfG¼ÛŒ?Z¡Sr‰"l?ï·ññÂíÄ?…Ì'ì£à-?>$a÷±ï?Qý«!öPx?jl4ё?…KÕã†=¿?ï.<qõj?'8æŽÚÞ?nFÐú?hÏ1Ï°­?–vˆçOܹ?Vn"K ?ïúD…mB?9uü¨´?)ðá¦À¾?ž9sa>Ó?@q±áGÈ&?5h·ü4FGL J1704.2+1234?ßò£ý
@=f°¦üX¬À:UÎyu6äÀ<E¢Ä»†S@'ê0µÕd@1wðÚÉ?Â#•ÜJÄ?µ(õÂå?ñK
¥uoï@
jŸHZ6Ø?îÔÎÞõÄ=¿êè±d'z¿Ö{%¥«ö"¿ä¤5~ç煿Ý@ˆ[XÁ7¿ïÿï0l¯AGNbll3FGL J1704.1+1234NVSS J170409+123421?ï®É¯î™?¥ÔDÁOf?TPFBíg?y§½7d!¦?Ã‹<^ß?¢ZþìÂÙ?ï …`‡?'PÚLN?BÇÀ¬+O¦?Q	¯–à.N?†Ïb'e(æ?'¥8¶Ù?Ù]é?ŒàË;{Æ	?räzFç?lY®ç6—?¢³)˜®?Šr]ü"õG?îÕۍïÆ`?™>jÀ9?jáΕòH…?U›£Yùg¥? ô*7¤ux?8‡h»4FGL J1704.5-0527¿æó°å¡Á@4ʂƒÓ^·À9Nµ×½Á—À;ΛâI5Ô@ =(Ɲ³°@Ga)Ä?®tÉUží쿕æ…ZZn?éά€§f@ý³¶P^'?Øø¾RW¿ã‹rX¿äÍhø¿Ûr£áq¿à×{ýQyð¿Í;;~AGNbll3FGL J1704.4-0528NVSS J170433-052839?ïDgÙEê?…CЅNb?RFf(f¦?K_XùňU?‰æ#üéxª?"R¹½¨½T?ï€KÖ]{5?ˆ ˜1 &a?S÷c¾'žƒ?b'ÎøSK?nðÜ>p?†¢öf	ï¨?îÖ9
çè—?‡Ææ._F=?p¶f 9^ß?fvðhéh¦? …¢]zJ±?†	ïµ¼?ìÖÁ|6?—F¾yß#?ƒÛçÃpG?m¶µ5K?¶Îw%á²4?–'š{³c4FGL J1705.0+7134¿é[ÖQI¸u@@úˆ?Õ%À;%J<d4À<ÍB=Jä@úCºÚ1@‹Ó"Qc ?Ë
ær@U?¿œ{Ì)8Þ?ò±‡Ìè{@]Ȑ'*?ïÒ(ŒD¿Ý*qB¸a[¿ã'<"pj¿à@ÛÈRé¿éÿ-!¡:x¿ïõc#»ÆëAGNbll3FGL J1705.5+7134GB6 J1704+7138?î­yêœR?µ'‰W¥?lñÒ9è[ë?cåÄo'(?£YD:‡µ4?œÙ§DiÏ?ïP!G³ÿ
?ŽŒg¥w,2?Wž¤k¶âÈ?ae5kÙw?"ìÂÄ°Z?Œyõ/˜#?î6þ'°?'ª Á¥át?}}ݪqŠ?p˜éR"¶Ã?ª\ö$b†Û?.7$q™º?î×KF^?\útkä?ƒtªñyƒ?h-²aNX?›\UAÄ÷K?}L»†ŸI'4FGL J1705.4+5436?澖iՏ@B~¹ÃÌîÀ:Õ3YɟòÀ<΂€x`d@ <–Þ(i×?üeћh¦³?ÈzxJB?ÀFí9Ô·þ?ö HZå?ÿ{=pxãì¿ëÇퟫ+'¿ÖŠmÂ%S÷¿Þ]*¸b2¿Òg"ÄËL¿åè4ÂTxÓ¿ÕpÏØAGNbllNVSS J170520+543700?ïx7"xÓ?9Ïô^?QÉn(îÇ?FÛ0u°f?¹	¡¦?€¯_·­'S?ï1ëd÷{?''+IñÄ?`_¿ë"'é?gèË¿½?—¶›Ž~K?è­&ìb°?î..éS)—?Áyc_tq?wÊ­—s£ñ?jŸø:¹i?ª#»·Þò?Šòó
1°?îH
Q_ÀV?Š´XnJ%?ˆ)‰\Ö?tÂKñœ•?¥tø"4%?‡Ä;_g_4FGL J1705.5-7423¿í-—ÛÜè¬À3jâ¸Ç\KÀ;ÏO?ÙÀ<Û÷@=ݱ@#oÄ8(»`?ùŽ­\Äüõ?Æ_šYÝìÛ¿¬6^ø?çÐ3:}ª@'¹Ëé"¿ïþƒþý¡¿î¨§ž¿ô!?ïý6âjBê¿âÏ@Î&i¿åFß•e?ù<a°@AGNbll1RXS J170548.1-742240?ï«ùôö?£8U3iT?-nØ&ê:Ä??øªK»š?"‹ÿ¢]Ù´?¢×u¿0?î_	éÐÚâ?·lIæ?dÓjª©o?…äÚôåd?¨Â*¸Gºï?·GÌÃRµ?íæ»p竔?'='	ÛrB?pÀg¿Eü.?fè'h~Á?¯|;ùœ‡F?'£xb¡Ð?èqÅÇmÐ?¹gs!ð%?o®éö±z?sÉ¿é¶-Ü?ͺ0Nâmö?¹|/Î$éL4FGL J1706.1+1000?ÊÅtFw@;åƒjƒ,À:?Ò?ÓT¦À<ãAƒX@¬åm¶@³@ÔÜeÇ?ÉȹAՍ?Ã
é!›?õf"X@ÙÛÃO˿ךLGo'¿ãZÛ¿è…tžtG¿ì3l>¼¿ïé!ACAH¿îÃøþ.ÂAGNbcu3FGL J1705.5+0948NVSS J170556+100006?ï»lbŽ@ì?~òYÖM?S¬à¡ô¸?Rp­èá"l?}^̀·
E?|a9¹öDX?ïiP*ì­%?Ž"[HÒ?Xñ[¼è‹°?m`1"°¬?'Fäæ›Ò¡?Š‹UŠ?îâ"ì¶?•1Ÿ0†?'•«šIÉk?udîö*?ª(¶ð.ÂP?'¿Ã8ƒ!?îَ¦'å?ƒ6[€ã$Ü?uœÌ™[m®?aîy(ÝóÝ?Ÿføhè?Å¿ÃrE4FGL J1706.8+3004¿Ø"'Œ~p@ALSóÀ;9ï•N±À<¥o@Î&@ŠM<žÁÍ@SÒDÛÒ#?ÅLLfn¿¡_w½Yoæ?ÜóD›:ƒŠ@ûÎíäJ¿ï5/øOó?ïþ¨Fۆ¤¿ì¢ì^b‹æ¿Ðì±#yó¿äC‹ƒS?³!Þ:øAGNbll87GB 170454.3+300758?ïyöÛÔi%?ŽAZD?YCﲤkã?St.ï2\?ŽYË')?3L‰nñÝ?ï¨%±@?ƒ¯®4DÚs?>Ëi «‹å?MØ¢‰qÖ­?…c†µ?'Ï%R›ÝÚ?íŒÉýº?••ußà}O?zçöôj?j-Ñ¢E?°2A˜˜¢ê?"J.Ýíå5?ïBhóÊ©?}DïNì9
?nälªØ?_Tß2´ü?"ïa
0u¬?zž#´€4FGL J1706.9+4543¿ã«
-@Bo.ßç[ÄÀ:¯¤Z½»¸À<_8ö@*‰¹QÅÅ@Ö#£s7?Ëÿ.^b6?¶~³Ë?é½ F@iùY¿Û^Þ&'d¿è-ÝvV¿æÐ
>Vý¾¿ë!°9ï¿ï÷á&öå¿ïÿöµšAGNfsrq4C +45.34?ïõí¦$ØÕ?f»Þós×<?-þ²ü?PØQ€Îm?PdÝVÍUl?_QŠ$ªrù?ï^`i
Ch?'|‰×?VÓ>HÐE?iY:õQ½7?'ƾú.–?"†Ñ?îÝ£ÊôÚ³?…Jü{î@ò?q-R"½?a&'é
fÐ? !fnd1?ƒw2	:?ï`·ªÍô?yi°ÀP?i؈g¤~^?V¬™æ_hâ?Á·ý±±Ž?x͖´+x4FGL J1707.1-1931¿ïދê4Ö@(ü)¥ë·À:ŽEîÑÀ<.·~†îœ@éûéd2@,p¼*¾?Êdk9‰äp?Øà۞KÛ@¥þ9Vbã@Õýê&$¿ï¿,Ñ?ïþÛ<Òf¿Þõt,öƒ¿á‹B=è¿ï›Ð`U*T¿ïÊ1¢ˆ.AGNbllPMN J1706-1932?Ì4c×NÔ?¼ÉÕH@&?Ü®zÁ7¿,?ÇEªÄ9Ž?Õëܙj?Č¸Þ¤L•?ÔBr‰¨?É"1Èß0?ÜÄچP&?Ì#ü®?ÍòJL®`?Ãgíýƨ*?ÙP8¸?±Ì¬ò)?ÔVý¾G?²'x?Ґÿñ€Ë7?°W9ʧbk?Ñâ÷#ì¨1?«$&®R›?×¾-`õX?´{«0}cn?ÖZJ®²bv?²cýu¢Ê04FGL J1707.5+1649?íø¡ž?N@>VÌ¢Ûa»À:4¿û-2À<L¡3ß@üÀ'a@DZ¢ãÅ7?¾¬W ùå?¾·ñH'$Þ@f´A»Œ3@
Ž~ZÎؖ?ïÿÔač¿âá',"³¿àêŽ^}
ó¿áŸv¼Ï)¿ë5â)>¿ßÙÙ«Ø`AGNfsrqMG1 J170732+1649?ï»[fjkm?ƒ:CGÁj¤?W€zzt~?`Š"Ù•?|r.,-EÛ?'8M.­ü$?ï"÷}¶s?ŠòIíxN?Vš¸¨k?d/‰àÿ?‹îɃ"óp?‡²(_µ+¹?¶‰É?'_DÒq†ò?‡n´Îp¥2?'M&:zÉZ?¡ÜGcÇ>Ï?‰‹ßºyod?î¶÷LMW ?'SâAa>b?‰,$‹,ã?p3Òu ?œ‹0Ñõ«?{ýBö‡-~4FGL J1707.9+0016¿ÒïÙ
!ü@6ü{þ~ÁÀ;‰‰¢À<D]­Z@¾@ Åå،s–@´ßbцp?Æy§¡D2࿔è:D')î?Бz{Ç »@þ=ìʙ?âziR©ñ¿Ø'-¿€Þã¿ëÁ
Áú᳿˗)gW}¿âòÅ_E4è¿Öi:@ԕAGNbcuNVSS J170744+001750?ïR…p£U?­¢Åו>??[ano­?3å);JÂÅ?•1äyÑÖ¶?l½Iô?ï¥r'N?†Tl#ÈÒ?6«cbwÌo?G¶a{Q<L?…íô@XÀÛ?…¹ü,ÿŒ¥?îKµúÅ6?'àuæq?k]ŸñÄ®;?_Ôtƒ¥?©ŽÆT"qÂ?'x"}gí?î›ÌXΉ?ßÅGˆ?Sâ8ÉhÞÅ?H3uƒ!íd?¥¯t'Ё?ÝUőƒó4FGL J1709.0-3525?}'¼59ð@ŽÆ±À9ºâP3À;wjš¨@uZê²@f'amÙ!?ÑiIºß™?׺@Ù$@Y¾L×I(?ûÉTZ[:?ïß(Ÿ[zz¿æI]Áý¿ãù±œÅž¿çޘÜÛ7Ê¿êMDƒ½¿æóï»åüAGNbcuTXS 1705-353?­RŸÆba?žKLX™?©›èW¿?¢¸$ê‰?ì' s?¬ÜËÑ°?Âim‡G­+?¼Ÿ0HZÿ¨?Â"¿˜æ©ï?Àå®aÒ­?æÜô·ôj9?Ä4Ncà?Ä
ãØåG? ødoé?õ;¯tï?§5 QïÝf?æøé»ò?®NÞùoŸ?¬nÀ?‡º.s.7?½|»"€Á?Ÿ~©Âö•?êá¯¯ÿ×? \Wygr,4FGL J1709.7+4318?ç÷LÔ*Jh@BÆâ¨eÀ8dVôÙ[À;ÑLF)¯ý@¶Ò«@Å}?Æ¿m? µ"â>?¸¦‹€¸]e@ŸAò×s@nE­ß â?ï¡Ä«–`¿ß!æúËb¿¿åƒC…¶ä¿äÓkL4"¿ér†áa¯¿çƒÐ¸ò$AGNfsrq3FGL J1709.6+4318B3 1708+433?ï—À¬×Š?‰£ÚinÅi?c®àošsã?n¡pƒåš?…$®SE?…QósÂBI?ï†0dj[?ŒX™£ˆ$?V?$O7ˆÓ?f?
çw ?V\þx?ŠÝ³Üõ©?îèGâ¯?'ðø&5g¹?~ÐUšE"?}غЖg?›HÐrI1?"GU6|?ï÷qÿøB˜?A0ÉÂ??+lE¡êÈØ?#Ž:aÂÇâ?K\î¶zëí?>Xÿ$±=Æ4FGL J1710.1-2030¿ì5»Ùèò¦@&°Z-rÿÒÀ:¥P¥4À<(äSÒ,@bBÁñ@ÐAÌS*?Ëü¨>O?×éw}e"@o?Rü&W@M™¢Rû¥?ïû´a"ñ¿åd8>4îõ¿ÈFû&§^©¿çŽâá·ª¿æ÷mT—1
¿ïÿW~lªAGNbcu1FGL J1709.8-2026TXS 1707-204?â{ôƒû¾?Ëá.
*ü?¼£?\}>~?´—T.šë6?ÓßGùظä?Á‡Hf(-?Ý(DDm;?Ð+㽨»?Ɣ‰±Ÿ?şMÆm±?׍w1¦9õ?ͼ':
fX?嘽*ý?®ï^}#µ?½ä8üt®? å~¢]>?Ì¥}œµ?§‹ë›•Pl?ÔD,³ûž¹?©¶‰NË]P?ÅòÙU£–?¬­CµU<?àa3P™K?±NÇuñl4FGL J1710.3-3943?ÁødçF†Þ?¦Bî"n%3À8@‹áJÀ9îÐè»?Ý@ܶlŽ@Ásûz_B?ºÉ³<ØÎc?Òê©â<Á@¶8ݗl@–f‹û r?ï¯Çˆp|?€œ ½­Ó–¿â‡ÐCyÒ¿èöN¦V@¿ïi˜¾&A¿ðAGNbcuGPSR 347.050+0.041?€<¤ó"Ï?xãWHžâé?á´«".ÁÉ?ÊÔLhï'?ÜÈÆzãX?Ê_‹'¹'?†í.Õr¡?†'|RCÔ-?ؐM®ú•=?Ã~ÐÛ(/Ì?ã\$pG_—?Ãp§+=,\?"êBŽ+[k?¼èwvCƒ?ã\²T)*?¸*‰€Þ²?Ø÷Ît÷ô?·ž0óC®h?lbꖞ¨Ô?[åf½Sàë?Ëà–c'Py?²µ²n?èëw|"Í9?²égõ‹E"4FGL J1711.1-4600c¿íEýœÅÞÀIZ¼äø=À9œR3©z¸À:µs¯ûî@ÿö¿ºj @i½@gÏ?ךŒàŸ?םŸQ>Œ@ÇOšr®@®ÞzIG¿à7(áÀ?ïÿÕ"[ʁ¿ê­ÂC±Ü¿èV° Ï/¿ïîõÁ2e?ï
•ö]AGNbcuAT20G J171106-4552548?áSž^"+?ɺ2u_ö7?Ò¹žÄ4,h?Ê
Ñ>c¿?Å>Hz–ƒ?Á˜â¨?ö?ºå
gåkœ?¹2'^àÂ	?¼Bsq"¶f?ÁûåF.?éDлÀ?Äëâm¶"8?ÇJ[¡ù?¤@Y|a?ÉìULh?ªÊq@C™?ã²SÚ¬§?¯â]¶ª®ï?¢¨2Öbù?ŽcU©³S?Âõ¨ðB9?·^ç(n5%?éô'–‰B?¸J7Ðه4FGL J1711.6-5027?åF/À¶#À؏>ÕÀ9Z`ȗ³æÀ;mcr–'@BDmÃ'@WS£ìó?º S7
?³'T®ƒ
·?øÂ+‰Æ@t&µ÷HK?µëî>ü-ý¿Û2¼`¦¿ê©ãÉh">¿â'¾@—õ«¿îo݈†Í?Áê}ø(p7AGNbcu3FGL J1711.5-5029PMN J1711-5028?ßEc²¼ì¶?ÄjÝ»ß?"›dq¤Å9?ë§RR4?ßpæ(Æö?Ä·9­Â?ãð'ö?É,֝ߏV?:ý°?ˆÙDN4òI?×¢Å
…ïÐ?É$9ãUê3?åê°Ëì—?±JR…ߎß?ª˜6	îø?"û¿¾m¯(?Ðח¨¾GÍ?®21S5?é‰ÔÈç¥?¢!ìvÒçŸ?¢Ho\­;€?‰|…4ç??ÅF'6õ? ÍäP¨!;4FGL J1712.5-3142¿Ô#ÓM‰9"@«½À9ÁöBçÜÀ;2H˜F@®Ÿ]'ùC@be+ÓÃ?Ñ|Òì™q?ØѡȽ@²q¼Û¾?þœyGêz?îÄ!ÝËLÅ¿ÔfˆË<¨¿ê§(-E³h¿å¼þùoÿç‹5ó×ӑ¿ïÿõ^'AGNbcuNVSS J171309-313912?Õípp¸{?Áêâ|qÞq?Ì:"æBh?Ãò'Í$Ì?Ûõ~|&Q?ÅòÅ;Dg?À‰Ʀ۷?¶iY
Æê?ÍTèí1G¼?ÃM"ƒÆ2€?䈀	÷#?ÂPê8[o ?Ì ë¦X?¤CšõÏó?È:›9¤P?¯S;d©?âìöþmV?°L]\o|*?¶ãµgÜ)Ã?"éØyÉ·T?Ëwøs<a?­âk¼ò‡C?æEÈç«°?®"¹­q¾F4FGL J1712.7+2932¿Äøà¤Î‰™@@t`$-À:HOžÀ<e$îÌÑÕ@ ˜V]¯³Œ?ümfL~?½
ãÉ­?ª$÷A{±?𨯠Ä?õeª^Ôê¿ÚIËÛ¶µ¿áh¼""Õ¿àXa@ß¿Þ~+ÿã$¨¿ÉI"ƒ\ì?¿Ú6›¦AGNbll3FGL J1712.6+2932RX J1712.8+2931?î'ÂãP["?œ¸µ¨š«?ms¼=%B?kíYEúœ?¤ü ?6{'?›ˆa‰ÁqÐ?î^RŸŒÛ?¥'Sù«¨¿?{1n'"µB?†
#G&A9?¦´¨5›º?¢°M³±?íWo¶%zÞ?•a5Y.ž?'µ2y¬ç?t¾[°HÊ?²íÜ$óz?"B;ëH?ém®þŽ»?¤EÈý"4?–Á³
QØ?†qؔEˆ?Çsf⻣ø?£ytè4S	4FGL J1713.7+8844¿ä1»iM š@;¤ß&k¤"À;Œ`b@føÀ<ìXJCðñ@!aTБÓR?ûNB¸â4=?Ðë}&œKü?Å4á^)V?öžÜd…@Ó~Ì
à¿ïÿÔÌuŽø?ïÿ®XëT¿ÅZF@+>¿¹\èä/"î¿áŠ!¡»Q$¿à…ïbùÊ\AGNbcu3FGL J1711.6+8846NVSS J171602+884416?ïÎ4&ÅPÿ?ppß\"r¼?HØlƒ y¶?AˆV5TÖú?uÊßãpá?nmxŒC7ù?ï"Õ@	½G?ŠÉŘ÷gÙ?M2†Šaû?`œƒ}ÇÕ,?Œ÷‡"ê"$?ˆ'rß$A?îêÆ?²d"C°ç?uêǟçû?`Fٌõ¸?«l'¸_¢?z "7R—?î³mÊb[L?‰ˆ'#Á½?sÒÙ-Ö?am{\Û!Õ?¢NÈ)ôj?ˆÒÖzMlI4FGL J1714.0-2029¿ïò½¢ÀèF@%4f+®´À:N{.t‡'À<
-€kË@#ÿåSƒ?ùµ(Ö¸ÞÙ?¾è(råЪ?Žtøì³?Òñ£[dT¾@	¼IGǕ¿ïÌR>[î?ïýð@o[Ø?¡K'_¯ª¿Û¼J~Sm¿ÑMR-Ê=¦¿Ê÷µP-ëAGNbcu3FGL J1714.1-20291RXS J171405.2-202747?ïsŸ{"ô¨?¡'t—_N}?:éIFZÿ?>7zeÑ>?'#œè\Q ?¡ˆÛ8Ú²?íÃühýÑ?¾ü|Vë·9?K0X¿·ó?f:"V
,:?±©¼úz?¾ÇÑUig"?ì18ü܆Ø?¤Ø¨‰,HJ?qn¸Éí£A?i%à«lÙI?½_LŒ|ï?¤¢
(¾õ?í÷=Ÿ‰´?úSžÄØ?c¯Äø`?ZZñçJ™0?·:Çò;ñÚ?ž,ÆØü
4FGL J1715.0+2616¿Ðªb® @?×a»úìÀ;ú61ëÀ<uÌÆ폻@÷ݜ¨Ã@y'½µÕ?̳€u†>ô?¦6ÌoÚ®b?ÔÏí~<Q@j#¹?£R~ÁÀÃï¿ä±À¢¿äþh›Œ¹¿â-t½l1¬¿ïþ*½ÃÅg?ïæ?šIÂÂAGNbcuMG2 J171454+2614?ï
Ææ÷žu?—Z˛>†?r&bøƒG‰?lÿÄϨìð?šŠbë_'?•ÿì#p?îÝʬ'õo?÷¥iŒ12?jTùë߈3?{³Û.(Ÿs? ~žÂ°€?š8ø;àN[?큚j
œ3?"ü)[t•
?‰¯ê؋	d?zyîÒÿv?°½/T½>?',©ò¶N"?î¤WYCŸV?‹Uº$ÁîÔ?p]¶+h?`/&ûSt?£®çµ¥?‰ÝÅæÆ1Æ4FGL J1715.4-4025?ÁÕ­Pۏ³¿ò"ãw3=DÀ9Øc—À:ð}e†l–@ x>fB)E@ð	yü?À¦Th-á?·vÀіá?ø ­Ú™>*@jÆ?ïþü—åº?íØ@|g°¿å†\Û£)e¿Û‡ôU§ÒB¿å"i£ÙŽ¿é»ÃŽAGNbcu3FGL J1715.4-4028PMN J1715-4025?ãþ)‰S'?ļWÔ§|?rJÄ:•?o…Ѿ¥?׺ÝÄpŒ?ÄÀ&<#å?Õ¸æ?̀àÀP›Î?}Ñî£R\)?Û™ˆí?äè¢8çÿ?Í)¼þû¢?à5Èõ¶]?´¹+ýü¸Û?¤}ˆiíCG?Ìžö6Ù?ݽ†êÞ?³ôck~:l?ډµŒ '?²)+‡é?©›.p>8?"ÜÉ ô?á!rRï3?²("(ÐÉq4FGL J1715.8+2151?íÎGfÿ@>HèÙrÍ}À;!•¥ïrÀ<Ž*pìÒ&@ó}Ë$@–U&£ø?ÍÕLù	ð?²8ÀxÅR?ã1&¹@(@"Üç÷öq¿ÆU±7pÉ¿æm¢À^ÕM¿à¶8 WäC¿èRˆÎp:û¿Í÷¤¼¸W ¿ï÷ÔCédAGNfsrqB2 1714+21?ï-3í¢üq?§NŠì©¸?]¸`!ÀVj?Y00\4«?˜}üI"lm?Œ"nH¿?-?‰½?–ù»Ž0?\ڔ–iàO?g0ӏä5r?œZŨ*E?•¹
Z?íÉR«®ÞX?"FyC£^?àe'¨?sמ÷ÕP?®òÎ`øµà?'ŸûÙMfL?îeÔX-¥û?Ž›pM96@?f›ëz"z?]g)©óÒ_?¨A`¾m÷?ŽTgõ´l§4FGL J1716.1+6836?ÓkZšð@@áOKD¢À9°›±¡ÎÀ<qD…kl@$´o#@ðçä€G¹?°Od´Ëy?‡Ç8ä"(õ?ÕòoÀ@X%åí°?¼]ø®§ó¤¿â'f$!Gx¿ç2bo¶Ç¿álÁŸG.¿è7®ø¦ok¿áº>À//˜AGNfsrq3FGL J1715.7+6837S4 1716+68?ïºéÞêUN?£nBÂýt‹?K´
mE)?fá¨;ºƒ?)'°Ã?¢÷þ¤û¯?ïÂýyŒ/£?|¤3…ü?6­)hÂ?Ke·Èù?}hi5˜£?z§¹Žîò?ï0/²Ÿž?õºOþ¤´?in•ªãœí?Za(ȄM?–ÌIÔO˜¥?}±<¶Bô?ïņ̃=Ó?FÍfîwæ?BèIµ¾‡?0RUÁÚÓ
?T™rŒ©x¢?C†åG¤4FGL J1716.3-3421?ïhʋ\ž@ݨ!ò™À9X™I—À:½r`o¬`@ZO+â1@¶Ú@¨?Ä'îÆò˜8?ÎÅ3æ·Yž@v§&J@¥Xz—?ïԋ/Ÿ*¿çÇb\«¿ÙÏ QC¿r¿å\½p8w@¿éÄ
¼¤¡¿ïý"#–]AGNbcuTXS 1713-342?Ç?ÛÇÙ6[?¶Þ\{Íà?´"æûœGG?¯àÃhÇG)?竬.–)€?¾Ž_@ã‡?ıþVæ(S?ÁZðÂHÿ?¼^¯npÑ^?½²kšgú'?çGª|x[Á?Æ¥þÒQ³.?ÏzÃs¤æá?¯½+%?¿ ùÀý¡?¡\oèÓì?ä=/ê÷#Ô?°{fÚÒ†?»Ó®ý°òû?‰þ>™	?±d™Æu?•6<x飙?êXöý?£fßbæç4FGL J1716.3+3434?¡˜ÙA0i@@Òb^™éKÀ;·ÀÌ
Š,À=yÚ6AÛm@[ N@†A­
ë?Ó¡Fnªƒ?ïþ@_‰Ó@9¥e¶š?þïΔ£º¿ïëiÀú)?ïÿæ4|ßO¿Ïàœøɪٿì¬Ù¢s1ü¿éæràÈ,T¿ïVqáÄ«–AGNbcuFIRST J171642.1+343856?ÄôÚûÂ?ÁĨt§q?çÛ¤¿öÒ²?Å܄£úz?¹"¸"rì?³Rq"†N,?ºEïÀs¬?¿o@¶Q?ê$TvN¢|?č†Zº,?´Õ]Êxk?¯'Û+i+?ΆŸÆT¥8?²4é×òä?ãŠÀ]šæ?¶º"®¡"?ÃN^Ã?ÂV?£ëXÞ\ö?¼´\*ëa?¦;¬7šÖ?ëd؊Qõ?ªaΦòâ~? I¿T™:?" JÍ1Á4FGL J1716.6-6707¿ÛªÅ0KLZÀ0Q€¡{kÀ;<MI^ïÀ<|ók@•±êk@<î?äž?Í/d\ m? j‹Üdî?Ö²Üá—à?þÌmŽÎºc¿ÒFr©jÈ¿ãIÒ±é¿èg
À²ã¿Ä˜†t¿ì!€ƒH¿ïÿîÝÃÀ	AGNbcuPKS 1711-670?ïìwQkí?'$ÃÉK/í?iZ2¢g~?`ÑQ"ýU?›×-/~5}?[s›Ö™?îõÉdß?ž­"Lýߖ?]v3FÉ)#?nö1îJ×?Ÿ†cž÷ŠÝ?Ê~gì@½?í·fá4à?—

¾…ð?ƒÓ\Pb¯?xÔÆ?v"S?¯"ºØ§F+?"?º»‹Zµ?ìÔ?'Yi½?š±Ñô÷ݟ?'fŏ!??së4]õßã?·*»Dù?š3þ4:>Œ4FGL J1717.3-6045¿íòM²1ãÀ)ížbV6mÀ:ïdDM6êÀ<•—rwí@6ƒºŠ*@mUhƓ?ːЇÂV§?ܚoÂۇP@=TT+
@jŒ¢:R¿ïð‹ž.SÐ?ïÂ{ƒ€¿ÖŸ§z­Æ!¿æ=í¡X«¿íĜý|B¿ïÿü¿ÙŸCAGNbcuPMN J1716-6045?ënM©ÉE?³ŸQïF?·èI–Œü›?¯r'"®Õ?©J'6Q¶R? ð:/h,?è¹Kè)?ÁýVä•}'?¹ú2mr?¶C>)3[Ý?ÀÊ•Ï¨¦?ºžrz?ú ?ãàïQ6Å?±àŒ€vb[?ÈNfJø?©2ÕP:Ì?È-݄q!ö?§UþS3ô?åFEY€›3?«}-^¤?L?ÃØßwžÉ?£ÙX@?ÇÕº…ôk?¤]SVc›r4FGL J1717.5-8114¿é]B;eÀ7^'¸#È\À:–@
²
ªÀ<iqDæ¹Þ@×`]bÝ@ÈCæߞ?À»¡VQp`?Ž¥vLJ"?Ììa<°à]@íBDH.m¿é
Ï@Åm¿Ù́»¬i¿ä I·¿à^^…¿áü¦¯+Ò¿ã!R•Ï	¾AGNbll3FGL J1716.7-81121RXS J171712.6-811501?ïn4ìAw›?ƒøû3zŠ÷?VüyÁ?Jíyj;¤Ü?É °@£Æ?ƒSó`?ïJ¶Sß?'—bVud?E¶µE_p?UJo€?–'ó5?'î$oo‰ü?íð?Ò¶µ?'y»!/?w՜Þ×ï¤?da~Ûëæ*?®ZÖù–³?'Yx߆|?íðÇmwÇ?â©k€Œ?q"µ?\îŸÆ
Ü,?®Ò.&Vê?î÷ûFW.4FGL J1717.5-3342?är‰lGH`@'ô}ë¾*À8:¯^&üÄÀ:[";"*Å@#ý:¨Èa@dc!7ˆ-?±LžŒˆ?Ã`à?›Ku@U£ãŸw)@4´g¦,?Ð87~òNg¿àÁQ'Ò­¿æl«ÅHg¿åðQ£"î¿ì›]"°§¿ã‹Ú"5¬ŠAGNbll3FGL J1717.8-3342TXS 1714-336?à[ìbâ?Ƴ"Ã…c?ºÕX3Á<?³M<¾zl#?ؓ«ªZIî?ÆÁc?ê؊3	á?ÇÔiµY¶{?ƒz½…ª…S?"e®±Ãr?ÆpñþÙ0(?Ç.÷/Èâ?à\|»€‡=?¸{¤mlëá?¸ˆ)¸íG?¢ÿ‡8½?Ù$üþ65?·,¹nðî?ß{"¦âÅ?·.Žj÷Ú?—ã•Æ›Ò?‰|k¥ÄnM?ß1ü³}Ç?·hª6g	 4FGL J1717.6-5154?²Q†È¤À "ön†ÆÀ9r"áÉ´À;x"íˆ.7@šU'þ@%!4y?½nýùëi?ؼ‹ ¯ø×@¯œ…×E@ 	%m¢Æ?ïû—áÂA¿ÙßND0±y¿çœ/`•Áô¿èÎ,~
L¿ï\˜AÒ¿ïš@¨f¼AGNfsrq3FGL J1717.4-5157PMN J1717-5155?é‡W|Êð?Á¤Dz÷¬?½0âñÖ¢?¹Vì¾»ô}?¶®6½Áß?³ò,ôráì?êõF±?¨.?Ã|+|P™?
¨þd?'¨$¯›;?Ã2|֔V?Âì>BÏýo?á:?"0?³lu®jÃ?Ф¼Õ»ü?°ÑW¿ÿ*ò?É͈ÇÇi?«s·/Mi?ëT(¸¿Ï?§cU9fø?šÓ+²$Ø?Œ§gè[Ã?¾ª[Ͳ¸P?¥
VãÁ4FGL J1718.0-3055¿ïíäŸ|\@7%€ÃÿÀ9<,†pÈÀ;Eˆ×ªva@–]Z#7@	•övê?º¿Œƒn_?µÎ–?`×Ë?û¼µ'•@ø§üaæ?ï}!"Î~~¿Ý]ÅB"пèw¦×o¾¿Ý*Ü·ü[0¿ç#ÑÌk¿çx×ì;AGNbcu3FGL J1718.1-3056PMN J1718-3056?ڕá]âÞ}?À7šÍÒ8?'Ü…ÚN)?Š!4Ôâ
B?â&/<ß¾P?ÀPF½Ú
‰?Ó$ëÖë?ÄDÍâ-Š?±9b5}×ñ?µ†¿Ž8Ó?äF]ÎCOs?ÅfjóO¾=?ÜÝîm?•?²DÐB3ñ?©OÙSà	?1çè•Ä?ßøhŒk?±°þ"¬ö?ÓòA±'kù?¨ë]³C2Ù?´nƒ²¦?•j$Fù±'?ãƒñVԓ¯?©"2™Ìð64FGL J1719.2+1745¿ÐH£>ÖKô@<†`ÔÀ8®j}L\À;®z¯É‡@B.'åue?ÿwÓv4:?¤ô^¿±Žá?¸??ŸÁëŒ@_e©Oð@"µçØí?ÐÞ;Ÿ"X¸¿Üÿ"Év7¿à!,jº¿àÑÍmÜ|¿âÎHÍÏ+L¿èÛÑLŽNAGNbll3FGL J1719.2+1744PKS 1717+177?ïڀêl\?dõ¼Cäzm?B¾'¾:?8í{"?pgÊ7»Žº?câT1
už?ïºyøŽé?€ ü)qÓ?BÝÀqúk?UqTŒ'Àn?€MÅz¼¥g?}Ûã5v?ï¡U?ŠEë*ʸ†?'Ÿ&Aåk?'†§¨Dšn?"œKtjúL?€S¬Ÿ«Ò?ïñÙ¤'u?J«:";«ù?w^˜¨"î?¤w§
'?[5AF‹'?JS«$34FGL J1719.3+1205¿å+ìï@9ØÈÿ¸²dÀ:Lí=…œÀ<4•äÙ3
@!; ¨×z?þ"ÑH\$?»1)ÑW÷¿™I#W›?àä†&ö@RgÎÆL*¿Ò亼)¿è	ØÆÖÇ¿ã9Pïܹ¿ÕõúX R†¿Ý±ª|ÀÅØ¿ÂlF9Ë'ÜAGNbcu3FGL J1719.3+120687GB 171701.0+121016?ï;;³Å?Šë¼ïzæ?[M`©,ò?NwfÙ§'Œ?–ã³|ʝ?‰Ð¹ô^™?ïY"…«?'>1Ö³?PÑvת2?\Àþ`ÚdÊ?"ÀgÁÏù#?'cÂ¥À ?í×()مx?"¢ñA­Ìt?uÑ̽¬ù?b¢h;¸æ{?¯ÓCʲ	L?'ˆŒss&?ìZUïw%?›ApX""?vܝ­µ¶%?gÓ˦DÍ?»¿†©k«{?›}.钭Ã4FGL J1720.0-5101?ë‰L
¹jßÀ‰êpKÂÀ:^Òn¦À;~1ôo@ڋIõ—q@À¹Ü/@_?ä/IŒ;?è?üÚ±'Þ@ g–@ý¦oëË@?ï8S~,UÉ¿ájzÈ:£¿éŽ¬ l¿î`ñ²_c¿Ûn€m¤?Vérí)ÛéAGNbcuPMN J1721-5055?Øι€–×?̈2‰Kv(?¾ÙÍ)ÔÄ?½Ñ¶Uºc?ßzӗ>sø?̇š^4£?ÕSà͞6?αFh(±'?ĝ€ø™(Ò?È…IQ?à.¯¸ræ°?Îۖr×áä?Ö³s>‰4?°¹Œ`¢Z?ÄËg)&£C?«+Ùv æ?ÞæÙ,ã/*?±žØF§^?Õx=>ú?º³6Ú3?Âå²Z›?¿Ÿ'U¨pb?àÃgóìR=?ÁÅ
ŒW>Ç4FGL J1720.2+3824?ïöù#Aùu@@̴ἩÀ:¨–ùݧÀ<pÍ_™Ä@bl¤CÔ@͘ÚVù?Äíañ34?µ>M˜-…?é·ýgŸKŠ@Ìٌù£¿âSQ¶«ù¿ÄGRºb¿ê"'úð̆¿éâi·S¾Ä¿Ò+A!]s¿ïûÜàSúAGNbcuSDSS J172010.33+382556.1?ïv¦ASÏâ?‹aªµZÀí?jUsvV?lÞhcC?‹¶N$ªC?‰'–Ísc?ïzôçÖ?Š)F5#3¨?Pš´äµ*?`åwR<×~?el)¨Ö?ˆrq° n±?íA×ÅHø?–âÑ¥m"+?'o¥ò³î?"—?EQ?±›ßÅPG?'¦ˆˆWXt?ï@ãÂîŠ\?~RÒxŽùN?pk^ù=c{?cSÏ:œ?"ȯãß[€?|2å+Ã4FGL J1722.6+6104¿â­ÏÝ)N@Ap\‰mÒÀ:2ì|•|ÔÀ<WÄ/oYT@n
I¯÷@š%™í|?¼•p•x?¶7¸¨þfx?õPû«©@8"XŒÞö?·äùibð¿è™‡+¿é‹K¿ì&+¾ß¿è!p}–ƒ»¿ðAGNfsrq3FGL J1722.7+6104GB6 J1722+6105?ïõK°L}Ÿ?KÖy,Ð"?GR¬Ç'r?D)Mäћ>?C~'ðb¿?>YO<N/?ïŒRzLO)?‰Ê§lî´»?IvIïÜQÅ?[šïÂieÐ?‹SüÍîpÓ?‡Ã³}†±Œ?ï+WZ"z?w,"÷j?o!^:à{$?`ñ*AÖ?˜–iM_¡x?€E0³X?樂ºO¤?pçé¿?jÒwzòTç?XÀ|ˆuÍ?€&3›ï'&?i§'z÷V'4FGL J1722.7+1014?æ7žõ@8M¤-fkÀ8ù˜zµ¨ÄÀ;ãn)©G@Z×^K9å@qû9Ç¢?ªc,u)?ªÙ¿4¢Ž?þáDŽO¹@!O[?ʋîظh¿á!—à¿ä99±Êé¿âwÜ{~¿å¾´`šI˜¿âgƃ°AGNfsrq3FGL J1722.7+1014TXS 1720+102?ïӟßpJ¨?žìƒÙŽ5ù?9À2Rú(?2!b(ök?t"tµ{Ÿ?žíKlÙéÈ?ï½O'™?~f,±«…?<ó*7f/I?P'òóÖ?¦¾´ÀÐW?|'ä׋{?ïvŸ6½?'á˜Nùça?p5ÙÀ5¨?b¹ª~naÉ?˜cµ©%B¼?€§RžZ?ï»ý¾	ì•?g{,ügWé?Y ¯ÿ3PË?Eƒh^¯-?{¸ôû<á£?e~€Ë']ˆ4FGL J1723.6-7714?¨ü:‡6À5Ë6žË2À8J¾*ršQÀ;Ÿ0µªq@¼n<c@t@ylÓh?Ÿ¡"
R%?¹?æàIV`@4·õ¥3+@
5"Š¶Ó?·ßW=ÿj¿á&B‰èK®¿ãX—Ü*7â¿ä'ô¦/ª¿é±k«¦·¿â.•3ÙKAGNbcu3FGL J1723.7-7713PKS 1716-771?ïf"¬Y•P?†%ŸTþ}?["¿.ûŒB?VZÄv@?'wÝ8?…"cß\/?ïÈ)l†œd?|Ø÷¡#–‰?=v'ºc߃?PÜ­ôÆÛ?zà'^?|ú×?îíB¦²¡{?'‰¼C¼î?…
1ô?…·%×3š–?—Ö¦('ց?Š]›A½:'?ï㈆£g?Y8Vº^·?6ŸXÔ|þ¯?)Jœ7èâ*?i¤	^Ìú:?Wìùu'@4FGL J1724.1+3304?ïEÎñ½Æ@?»XK±À;$Ÿ¹šÀ<¿Áõv@ÄÑÞ¯xS@ȝ»gI»?Á××WjJ!¿µE@¦ä/ë?ï$8ž×ñï@½´«î±?èÚ>Oq¿î|b¡µÇοÇY¨‡s&¿Ó³ä¡Q¿á'óU͒¿Þj~yÊAGNfsrqB2 1722+33?ï0ãa¾8?³D^]â¶é?p[Þ:²\Ç?
ùÃÓ¬?•Ìœ9Œe?¯üþvr]>?ïz÷V~¢>?ŒM§úÒ¥ç?K6‹@Ù	?XH{§Ÿ?ŽÁ¬U¢¡?ŠÓν*ە?íéä°ÿ?"ÉkanÃ?yºD:%?rËÇû5Ì?®6±Ìh¼@?'srœ`^Ç?ï5ùä´¡?Ÿ¦šÉ­?n[íŽ!Ø?`"WÏܬÒ?•u_ËÎ'Š?}kkJìèî4FGL J1724.2+4005¿ßTãéh@@'dobÀ9biAâù_À<RS‰êÐ@fëÇc×@§Ös>»ý?°ô¤9/Ì?ÁÔÀa.™@döÄíÛ:@Ž¦‡é˜à?'M
`!)¿â~€Ǒ$¿æ@&`¼Ù:¿ç—áìèì`æʤԿïýø‰9™AGNfsrq3FGL J1723.9+4004S4 1722+40?ï¤ø:¹õ?IP9@¹?m^œÎK¡¯?e›Q‡	5ä?~Ô«{}5?xÑx—Á5¤?ï¯KëôœI?…à÷Ðփˆ?@ÀÎl‰?Sïˑo¬%?ƒ ø?"â%…†6‰? ûö?…ó*×°?|	š0­R?q]ÿÎÚO~?—í%UÍ?€ÜFÞYS	?ïê¥æ	Ð_?Q TV>?:Üêþ¢?*(VxNß?b>XÏÐÖ?O}µuÄD4FGL J1724.2-6501?îÙW	Q7€À/Ç$ p¸ÐÀ:¹n$ É9À<DçԐ@8O§³
@ê/~r̦?ÅÕ^fWM?£GPCۄ?Ý܏¸oH?÷<í–ÆÖi?مâ,°b3¿ê~íEé]¿èS¤Wb½d¿âr‡ÂÀð¿ä÷ÞþþxA¿ï뒠+.,AGNrdgNGC 6328?ï{y¹D?•ñ'}þ?[Ž¨÷V±?Tïs쀢Ñ?œW¯nH›?•lß^›f?î]iœj,:?©YcRl?pˆBÀg"?h%a5é?¨]áPKê?¨_€#Ç©µ?íqÑJçÞ?•VøJH€­?"|Ø,å{?së¦àëó?±è>p?"ˆHŒµç+?ëd$Âý?ÒÅ Ÿ@ƒ?–C¤ŸnY?'JÌý>²?¿N…²*~?›'¹THƒZ4FGL J1724.9+7654¿ÒãÀ™¸£J@?9¦ç_ö
À:¥ìeïH"À<^n£KÊ@¡@-lŸ»@¦;îך?Å0‹x™™Å?Š,†==ŀ?Â{R'L@	1‰èv¡r¿Ö5²ÿÇ ¿ç$w®G¿é¢
qÊÛ¿å`ø0'æ¿ãÔÄ}ròf¿ïÿïn¸D€AGNfsrqS5 1726+76?ïßnTÜ?fèa&!ÝO?Nº%<ÆvŸ?E­ó¿äÌ°?hãW\L…#?d£ÿ9E?qÚ?"+^œò?@›"	-'H?QÁpŸƒßü?†jz6 -?ƒs" y'?îþ³kI?ƒ—ä
G´?kÿþc.Ïñ?ZR¡Ë /ô?œ½©Ò¬¼ø?r–;œ@à?ï"
¸š‹?pÃig)^c?ZɁ³ÛÆ?F¾Níɹ?‡à]ä•?p;4ö
΄4FGL J1725.0+1152¿í"­éª@8yLýÔ»À7éÇ88U²À;*µ[–ÿ‹@°\ô͜Ö?ü@—"ìck?ŸÃËØlNn?®}£;P[@Öâdä†'@
s—ý7N?暴f¶î>¿ÝЎÃ|Áò¿ÜWí'?2E¿×QDX­¿à"$݅Û¿ÝÃÎ ‰ãCAGNbll3FGL J1725.0+11521H 1720+117?六ßW‡v?€ÎÒ÷s¢e?LÃjUóö?F'96µP?"OQ"¾ãW?€2^cî"?îƒOCˆ‡'?¤èŠºÏV0?'uŠŒóo?íåê1@?£#®dÔJ? ~֮ŷÚ?í\»Û±@v?£5Z,"‡?‡™‡53؃?'&Oaãæ?²&ð;ρ@?¡¨#­ã½Í?ç²·èt&]?±»ôÉÀCš?ŸÀrÁԅÌ?‡?üNÞ¯?Í=ôÕÐ?±è³úpà°4FGL J1725.4+5254?ƛÿ~¿'k@A
ïܜM©À;°£µ|N/À<Ó¿jäz@ ¬Í÷ó—@"0Ÿ<¦?")JÒ¿¶9&ôŸ?õe=ð%—@ŒUðLƒ¼?åãÉjÉø¿ê¶u¨"ÉY¿æ­}±Ü†~¿ãÅ6jö ¿Ø6]_+´¿ÆŽån.\AGNbcuRX J1725.3+5255?îb¿ËŽOœ? ?è.áÑ?sÕçüVæ?ló/ñP??§YFG™ûo?ž£­¨ÿ?îrSb=ò?£Jò……!ã?t³7èüŠ·?†ö¹¡ß‡?¦Dbß¿?Ÿæ3lˆ-O?í"C›ÆÉ?"ß3É;®?{ÈúOÝi?i"±!ü?±¡S|Ëàz?'ëìÖÓF?ì‰Lð.¥N?¦þK"'&Š?{GòN¶8O?u_EƑ[?ºYŸr?§('UÓë4FGL J1725.5+5851?ì¦ir@@üšõºÀ9ó+w}À<'\ä¥6@O²×-Mì@g­Ãó	w?±ñOŽÀ?žmã;åŒ?ë?N_¤@-2¢""ø¿àžóu®¿ácAM¨)¿äļþ"°.¿Ý»¹^Û؃¿ç
ŸàÛwŠ¿áM20±ÏAGNbll3FGL J1725.3+58537C 1724+5854?ïç$ÿLdô?dÙPæ¶T?9"ìlRo&?090ÑìË%?eªc&¾?c÷uÆÜjâ?ï½FG½¾?€"ùÔMœ?;ù¢Ð¶?P0ÃjÔó7?Óóë?}à…ÞO£?ïVJj†7¾?w´ðèѓ?cœGÿ´Z?PbFº>?'Ã)¯B…ë?uÓPý¹)
?ïçDFú52?R´ÁJ¬í?KŽ&+´??7{CMû€?aؼ?á8?O}÷•ÿ‡4FGL J1727.2+0644¿ÞàŠ†x¡õ@5ÇÛLÂPrÀ:†R{ÍÖ¸À;ݗkÖ@ޛÇÇ)u@—¬úŸmï?ßB"úùZõ?åðBrÁ>?ÿË.LC¥q@	$á‹Ë¥°?ï/›™N?¿Ýsdѐ׿ëmµz °¿ê3­Á錄ïÿý¥\Æ?Ü×æ¼5CAGNbcu3FGL J1727.4+0634NVSS J172720+064123?îÒ¨MÜB?¢;æN!lÕ?ƒ÷#lл?ƒ~…§_ْ?›¯n¤ŽW? ñdfù?ëôƄN?ì?¼Ì09Z
?§8DYk?²I9Öþ1é?´½©±ña?°øÛ?ê'Øßù¼C?¦ŒwÑ^u¾?­>òbîúÌ?–û4˓ÂO?Àßç]PC? ü§¿åJ4?é -,Ö5?­S†5@¹Ç?"Ÿ	ÚX‰Œ?p}‡fÛ?ÈëjL•û?¬SÓQ54FGL J1727.4+4530¿å±P"t:Ý@@¥‡+À8qq¡-ÒÀ;ÿ+Ü&Üä@Jž5àŒ@'eŸ—
? p·ß;¢?µq"Q³ÑÔ@?Ø2\@|Ë¢Ö.J¿È+ç—rx¿ãšG>'òŽ¿æýdQµ¿æ­ÞÎW¿ë#Ÿa¯g¿ïÿÍ'ý AGNfsrq3FGL J1727.1+4531S4 1726+45?ïãÛ?~™]è<ãc?qX+1µ8?fúb7͙ð?¶vBÝF?z0̙KÖ*?ïFC䜽?¢x§Žåt?[¸ùïÞ,R?k`WI¶Ï€?•rgän…?¢!Ÿì½'?ï?u £?Œàà8Õh?}â´O*c?vD JT-@?—ßdK¡eƒ?ˆxcøö?ïòM9?H²=ˆ=ø?Bo–`É?6l3t¸g?R./•Œ¦ƒ?B'e¥¤d4FGL J1727.9-0654¿ÝÇTÚÅ*c@. ½ì_9KÀ:AíHmÀ;Œ¿®Xë@±F ù4_@Õ%t.?Ë*"<m2?ĈSvÀ5?ú§ÇúÕô"@V½sé[Ï?ïýª R¿æ‰ùž<°¿ã~ÊuÚw°¿å¢>ƒÉN¿ïõ}$îÌÒ¿ïë%@@AGNbcu3FGL J1727.6-0654PKS 1725-06?ãᒱ7P¶?Ç8)l"6¡?"xûµÉ*?'Àµnö0?×Jìv?Ç%—žRE?çžô!EdW?Ä#<šNP?°σÔ‹?²ÉV'Ç?ɂǹ_a?Á5¿Åí¬Š?áÕòH"?²`Ñéý?·&~󬯓?¼kËmõ??×´^öBò?°óñÍâRk?ÙÑj4¾?­)þÖõe:?²séˆ÷5§?–üÀý~•?àÈÍÄXþí?¯VÒJÄq4FGL J1728.0+1216¿îÜ(̹@7ùSÞ¤e¥À9,ÂËÂÀ;Ì4–	Â!@¤é
ìî@qÈâ\?±\Á! ?·›‹¡´EA@³¼?¶Ï5@€'4Í<3¿à#Cf‡–¿Þ
D<œ¿æcˆ€l¡ê¿æk:ÁG¦¿êœ€iFëw¿×ú ø2¬AGNfsrq3FGL J1728.0+1217PKS 1725+123?ï¯ä®w?€[œàzë?X›¸ß0X?P'·Â?€ó"'}<7?~Ój)®AQ?ïï*hœ×?‰4úYï?SPk[3S
?bürþ?'úr_'?‡u$:]?µ8?Õ]°l? Þ(H8ª?vøméÐf?¢ž0Zšhß?‹™ZÄ¥;y?ï›tG˜?'U0D7Å8?vG°>Ýx²?a¬M@²?˜š¥gUž(?€ƒtí̤4FGL J1728.3+5013¿»f[ã@@ÄÁæ¯ÍÀ8'û¡ÌnÀ;·–5df@ Ïÿ1N?ü%Ê_4Bþ?Ÿûß=#?ˆæ2	Μ?ê{`ž{V@Â
Җæ6¿äŒšþ§±¿à:þƒ©¿ßý‡[ח¿ÐþD4ã¿ßlL#Å&¿ÒèoÀ';¯AGNbll3FGL J1728.3+5013I Zw 187?ïîÝN?<Ð?mè½Úµ'?#ö¾
$f ?5˜Ô¤¬?_ƋÀAÓz?k‹Pè9?ï¸AÔ$Ðõ?~‰Æ؆ú*?=²¦h³?RR^°}+h?õÂÀ}F?|»rñ…ƒ…?îõ
æ)öA?‰üÿÞÈç?hsörË-w?a™lý¦5‰?žOÄlgÒ-?ˆ­\%e0æ?ïã²JØé?Yòì²eøl?%ŽŸ+"—?FŸì
E?jûÍ4e8?YE`ÛÉ4FGL J1728.4+0427¿âI>'áy
@4w%_5½À9†…˜ZÕ9À;®MnGÜ8@Øõ¥@x<¢G¾?¸á(ypÚ3?ώLßV½&@Q\þØ<@Š³áŒ?å÷$+Ž¿ãs…ô¡'¿èc¾yå¿èA~O'7Ë¿ïéÈ@K·¿ï¸ 7­ì7AGNfsrq3FGL J1728.5+0428PKS 1725+044?îqÔNÌ»?¤û–ÞÂY? °¤U=Ä?Ÿ§c*ÞÚ=?'¨ݾy?"4r"$½¯?îRÑ¢\õ½?¦`uˆª?‰<˜	b
,?'Ì6Fps?¤ƒ¿×Ø Ï?¢Z­E^\?븢¹ª¤Ñ?¦þ¦9Ÿþ?­áï`c£"?œ5p¬†ý?³Iò'yô?œRM҉–?êÕõݤ.?ŸWÑäý8Î?£\¥çþ?‹S K-ë"?¿¡þ#"?›Ó¦ï14FGL J1728.5-7303?éÕ qMÀ4$ýó¶E¢À:Hä.bÀ<3+†–‡–@]îþOý@†Yùp™Æ?Ŧy{ìài?È5>eÁOì@Ü¢,æ@io‹þüJ?ïò';׿閗†™â•¿çÙ­…ߨr¿ìƒ[i³"¿ïͪB^Ia¿í³ð\ôÎAGNbcuPKS 1719-729?îì7ÇMw?›ž>­	¤?àf5"¡?€ÁXÒÕ!l?™ˆê{†œ?–ƒf¢gË?í³"W!øG?¬åœáºîÍ?­š ¤?›ÚƒÆŸx?¬¼sÆkH?¦¢(rq¯?ìm>fV½¥?¡#,
™¾à?•óâ®°?"}³"?·UÔ§?œÂǑøP—?ì±õWk?—³àìZ?§"gªà(?Ž£MvÁ¼?³P<Ó4›?'Á½Nú_4FGL J1728.6-7448¿å
¯£ú¤)À4ó*®)s—À:ÄÎG÷–À<QiQ@Ã+Ìa˜@TÔ#&v?ʧ¹"ÓÝ?Û3ÿµ­K@LÛzåy@
¢¥Em(¿âîó2'#"¿Æþž–ƒ—¿åœ¼™xâj¿írJÀm˜à¿ïÿ—?LF*?à¯:ëŽYAGNbcuMRC 1722-748?ï2†±Ø÷¡?—gص‹?u[<·IÏ?wÑsáVŠ?"XZ—˜.?"Qcü÷Qå?î.ó@©*ó?°"N?†2È?ˆð^éÕW{? Û0¶O?¦Ô´:÷úó?¨C&7?ë?c¤²l?¥*3êl?ªõEA@—?"M%Åó:‡?¹»b[9ÌR? YB]Å°?íÊÞ¬Ñ|?•¦§Âݞ¨?'Êa—‰Ž ?ppµÈ<?®Ÿ|ÍÔM?"?¼,<Åv4FGL J1730.6+0024?Ì®ƒ>¿@2§Å¬À9;z6'À;¹ö&bjX@|ó€À¯³@«NoÑI?±Í .ɗ
?Âòø-}½@ìÂ
V)Ø@Ž»NöY?ï`8_¿¿ÕmÐ}†h¿â}»'!­Ð¿ã3øŠÀ¸Â¿ås•¹:¿ìEUt¦›
AGNfsrq3FGL J1730.5+0023PKS 1728+004?ïµïƒ¢ï?wÔf?ï?^AÛ	&?V+áF^§?}wǶl"$?t‹æ9ôÃÒ?フø驼?€vû©|?<jn»þ~?K÷Ϗ%1-?~ùä?b¿?Úzçß?îfâS¨Œ ?•ÌW›jõ?ÒÔWN&?†YF¦½A?¢%¯£µl?T<C:'?惡®§1?quhº?ImlƒÄĤ?;¿KÇ´Ûä?"º½Ž'W?pûÑ:G¨4FGL J1730.6+3805?ïþ²Åå|ò@?ŠDØw$ûÀ;u¬Wâ?%À<Ìè^ùŠ›@!2ÂÄá
?ü `'çα?Ôy:éàÙÊ?Ó1¹KÈË?ü7«bï¹@´=«\9½?ڊ#¥ ¶Y¿•sÂ^M­¿Åûá¸AO¿ÚÒ²˝"¿ÞødÓiI¿ïÿîͨ"ßAGNbcuNVSS J173044+380452?ï~‡®9?§Ì&鶏?XØo[vŽ?X/
†K˜B?C°Ì"?§ë´gY?ï}mï?—'¯nå¤o?eM°¦Å¿d?snL_›™?š¦¨}"Ê?"E*þk?í"1i³³Ï?–s{·}Y?‹½¡'ßë8?'ò#ý ?°fÀ€&d?"–CñurÉ?í}k¼†?˜1"äJj™?€œãš¡ˆ¡?qäA÷&À£?²nÇ¿?˜ŸÕeÑ_c4FGL J1730.8+3715?ãrO™¬u%@?WðgȗÀ:NqªgG7À<ˆ}@@úÈi»°p?þ>ΌÀmC?Á×¢é¤sè?Ç=×&ñ@R4ebZh@)ߥ¥^?îìPá
¿æèm<C}-¿ÕÞ½ÛB[o¿àÞYçþ¿âš8%
|¿ïùK ½OVAGNbll3FGL J1730.6+3711GB6 J1730+3714?ïÂMjYm?qúgs=Á?j<9T¼ƒr?c"Χ4€?q»` u­?f­æ–\?ïOŒÍ'ɯ?ÚJæŽtA?`{¤Q²?iLð›ªú?"þñÅp†P?Œ{a×EÏ?î¾é&Ð?Œ% ëÁò,?{ƒz͏?t=ë˜ËÖ? ¯?mƒ¤˜?†i
™Ô´?î*½/¼g?ˆ«N3Õò?ŒÍaØkÓ^?p&B-¢?§Ùû¶éD³?†'Yð˜ç4FGL J1731.6-3002?èyÈøú·?ÿ'¶@™MCÀ8èšÆÀCRÀ:ßPÃfò}@÷–ýˆ•@HËwb?·Õ÷ÃÆhÛ?ÆCž:h0Á@
uÐfµ@¿@1{ys‹¿ïþ}êªr?ïÿùJYQ¿Ü¶ûª¿ãA¾qg¿æsßVø¿ç£5ÄÝëAGNbll3FGL J1731.8-3001NVSS J173146-300309?ãîÑn5?ÄU"ܳ?«ŸsäOä?£ÖcJÊÝ?ÔÁÐo~™š?Ãs3k"Ø?ۆkš‹?ÍÏQïë´?¦u½â"Ix?³v+ÝñÍw?àÕnT'/^?ΒvwbÃ%?ÝA)"Ü3{?´ê+xLÓY?·þâ»'? ÷W*oôW?Ü¿V´ì?³^µìåÓ?וu+6F?³u旮sÞ?±!µ¢åY?™/ÈK6þ?â@!ö2?µ÷sR
±4FGL J1731.9-2719¿£7p'`֊@GëäÀ™À9-	¼AdNÀ:ßÀú)&@š¤Êû'@ØDŽŽoš?ÀÙÈ]ÒC.?¬øæÂR†œ?ñtŒINþk@{9ºHf?ïÿMB}þÞ¿ä/½BNF¿åA·ZtÀœ¿è,›Ÿ-WQ¿ç?B5.µö¿ÏDxjtèàAGNbcuNVSS J173149-271928?¾Éw†°?°å¡͗L?*¼âJH?‡ÐE	…=?ëÊ;݆ÎÀ?±ã"o'½ô?Ì­ÕbÉ8×?Àצ	|?ª"½£f]?®3xÔI­?ç+>ÍOô?Á«3»Ë»?Êŝ7R›?ªM_û‹H?°èË¥f!?'k‹'¯?ç1–F}~•?ª"_ Lµ?À9*Ù÷'°?ž¬‹ã°B?¤Â'•bJÝ?Œ/:}cCf?ꥍ +ú¦? énT¨aä4FGL J1733.0-1305?ë{åäc–@%;À n À7†€Ǒ$À;
ì-4ì@õ ÿÿÕ@ُ¨?›dN^1ä?¿~™
,¹G@"? §?@žáW¿Á¥ˆço»¿àãÀ~౿äásLþ¶T¿ä.×N0¼¿ê:ó¼$ÞÝ¿ë.HG—nFAGNFSRQ3FGL J1733.0-1305PKS 1730-13?îÓ°Ä¼)?¡ º¿+j?}…ΛÛD?{îšO,Š?£B 8Üô? Y–ÄU?t3‹?°³¼"ç«?r€2`lI?†.óBÿû?¢íÿ,¯>*?°0š ýō?í½0§ÐŠ? š ±"+?«v[ú-?"ÀU7?¥¬¨šTú2?–{Ý¿o®_?îø÷¯xÈ?ÓÇ;
"?vÅ<
Þµ?nî‡\¿ç?›/»
¾ok?Š;eÅüèÖ4FGL J1733.4-3943¿æ§ZìÀí·ä{õÀ9cßÏpÀ;oÅYa›@­T9éç@–-¹v®³?¹œRÜpÙ²?£dûØ(¯?êúâm©Q@p
xä¿å îؐO?ãæóŸI†Ý¿èä^ÿ"Ë)¿Úâ@|q뀿æ¤0ÌP¦¿×@êÁTs AGNbcu3FGL J1733.5-39412MASS J17332704-3942172?ãû8¤Á©½?Â/F%	¤œ?†TĶéþ(?¯ˆ‡¼Lø?×VèÅ\"?Á}8>äp?漕B¾¿¢?Æž­`"?_Gc8B9?r
‡AÌ¢e?ÒgÍ3Hy?ÅáÑ$ù?ã²û`%^@?µT'¼ãÜ? ~ÜS1¼?‰ãW/Ïo?֘d*ÝG?³åsrTlÛ?èºÃ´f?¢»×/zt?–§l¥³ ÿ?~	‹)'à?Ê@+6ÊG?¡òÅ"Q4FGL J1733.4+5428?ëÐZ—Á@@vÿCAž0À:"Ž÷À<m‰5žG~@MTùLˆ@å!ÂÈg?ËE'Á(?Õù"›…¬þ@ I@¼?øÜWYX6?ï,B³Ù¶À¿àáô±î$5¿ìÚ _†xU¿é¨¶7_޿á"Z¿ï÷ö'õ;AGNbll3FGL J1731.9+5428SDSS J173340.31+542636.9?î/ÝìÜË?«µq/©	?ž†'8l?§sÓ|Š?›ƒG›Ó.?—s6Ë\Ã{?ߢõü¿K?Ì´¤=Gƒ¢?×DìD‡n?ÌýO²ožè?Â0;õøâ‹?²èùJÅ¡Â?çx.Ò»|?«ã38e|?¸lúx™z1?ž–)‡<‹Á?Åç†hT÷?¤³°Mpãà?ޟ­ã¢?´Þm'B)Á?Ú¦ÝgQX?·‹Eã+?ºèm:,?œÎ
ÞöE4FGL J1733.6-6054¿ÉʞƒRJÀ-{¿PãGcÀ:÷8±!vÀ<0Ò­·]Ð@\U"°K@°h:{üÑ?¸ÐW›ÈH¿}Ëg<½/'?Âø4È4@+Y%¯g?B`Í ¿Û:"dKY¿äêkäT¨Ï¿âôšÜ¸o¿åLã=Qš'¿à•ªA°sAGNbcu3FGL J1733.8-6056PMN J1733-6055?ïÌ´<>ƒ?ŒfÊ;Ü?Fpνìå?<i"ñ+?w+Œ
#<?ŒM€§Î,ß?ïő¡xa½?'Ѝ7ƒƒ?*µ¿åÚi?NE»b䚩?|aD P?%§7ê?ï×Qì4«?'O‹ª(¨?n'b·°?_kƒ±ê¿Î?› )~–ÓŸ?€C"ÖÝY?ïtÛûïD®?p®B~ØÃñ?^±*ä9ù?E¶Ä€mf<?ŽòÛ§›-³?oû–WæŽß4FGL J1734.0+0805?ïý-&Ì
@4Ü^³¾#À:{÷öFCÀ;ïÁ¸œ" @*¢Ø\¢î@'¤ŠŽd?ЕGûAT?ÝûÈ£GmR@·üƏ›ê@ç‰>W©Š?ï³Ä¾
'¿áî)°•	¿è
¼`îØ:¿ë\4-n¿ïÑÙ|¸[¿íññIƒ×AGNbcuNVSS J173400+080628?쏉ZÙªx?¼tv$¥–?¯»úZåa%?±aÒ­¦ ?§Ko÷÷N?·:@)¤#5?ã¼(Í»?ÊTi¹hjû?Ðä}tIp?É)"$Ö(Í?ÂԈt67?´¸¿J¼]X?æf*þa¦?°+ndݙ'?ºxDH—'? Ly쟂/?É+1âkã?©9Jµ`:?ØÇ
ÉA+
?«åÖXoßB?Ô(ˆç¼E?±I,I³–?Óm'×°?°Í-3."4FGL J1734.3+3858?Ö¨횀R@?%á;ÛÀ8B9ҍ×À;¦ôlNô@`A–{@ÓÛÝr?òq»ÈÝC?µØçžp*@S,ü¸Lã@âà‹OÕ¿ÎAØi¿àW-^T¿äi\ð›Þî¿åÜ Ýp3¿ç½ŠÒS¿è§"ïQ0AGNfsrq3FGL J1734.3+3858B2 1732+38A?ï²aŒ$¸?uê¹ñš7a?JÅì	—-?BŠ¸Öeð?»>6fX[?uo'ùf¢?ï'mþU[?Ž¥úë¬OÊ?Q†µC:?aՅä<.?‰KMÎbG?$}˜¿?ïd[kÀdÇ?~oÓFJß
?m"(y»¹å?aÅ(¦'c€?"Zñwߪ?{	7ôH?ïóÜoaó?IºÎ˜˜?)é_ªEš›?  Æ®7XD?U
»+óhÜ?H£k"öŎ4FGL J1735.4-1118?Ðàø0†c@&p9ïôÀ:J­£;ÚÀ;Úv¾£>^@ µ[ÀE*@Cò%Kéã?ÂÍ1÷sê^?°
$àÎÑ#?ìÜ蹒]?ýiù¿Ê?âå=¿ë]ãà刅?³¹" k³¿à!ÑÁ©-5¿ä¾µÅ$b¿Ü|ö`D
vAGNbcu3FGL J1735.4-1118PMN J1735-1117?å2Ùµ‡I^?Ä:m€ÿÌJ?ƒ²"Ü?w3ÆWù<Ð?Ôü¼[à~e?Ä:9f¨.ý?à˜ã`N¸Z?Ì.ÇXÄpõ?'㸥ŒÕ®?"ßœ¥ñR?ݯýµ	Áò?Ëö©¼µ õ?èÁóØÿs?¬·sB‰\,?žE–<¶?‹˜Ç#è§ù?̏}Ôkp?ª'¶ÈYò`?à±Ï6¢u?©Ÿp‡4à?¤âT/O$½?XßñÈá?ÜY¨Ö?©ÕÙlÅL»4FGL J1735.8-5932?íLRÁv¸À,™¾ó'ªÀ:'çIOÕ*À<8pÇé8=@x/fŸò#@®œ£9UŒ?¿ZÝààô¿¢Ó›À\ÉQ?çGžÑÿ@a±"«É?ïòŒÝt¿éå»±–¿ê©bdy&¿Ò(>"$˜¿åuöâJ"¿Ý‡±d¼m.AGNbcuWISEA J173553.24-593204.6?îÿ³ÕÝݐ?–¸YÂç>?p¥1ëkÎ?gh§lÜcÄ?œ›÷Ér÷?"ãn9©7?ï½v<?¡Ê¥ì°?TKkŸP¹?_>Q<#2]?›ãš'C4?¡Ž52t?ìúôÈt?›ó²ÀûgW?Î",¦
å?pLr°9?µî›äú®?š"ˆRѽ?íJÐ5,'?•³=¸ˆÙ?‡éfú×î?tJ,lƅÛ?´¨|Ÿ÷?"Âm÷±8!4FGL J1736.0+2033?ïÙÂ¥Æ<@9kÿCAžÀ:yÇQcÀ<4¹º¡Q@`Ý•.?ûåå½^šÀ?»%33^&?Âڅ4-@	qá߃ˆ¶@L¯d‡/¿ÞTÕDj"?ïùînD˜¿Ñ0oço¿ÕÊÛ[	T¿áþàzÿzŸ¿ç#pvóÒAGNbll3FGL J1736.0+2033NVSS J173605+203301?ïõ—IÕm¡?o£…ÍM?E:ÑáU•?Zœ5^3?DhÉ,&é?b˜±4…0?ï²C†ß½?'6ÂÒª$™?F#vñ©"(?\©ClQ³í?'ç­w~?€dLþ¬?ïenòK÷?ƒT¾7—!‡?u'²5Ã;Î?r†¢¿…Q'?—ò¥"E²,?|˜‰ƒN@?ï€äCf?tVFEqJÚ?aa¸ŽHšK?Q:½W¿eš?‹nË¬¿²?r•Ê £o44FGL J1736.6+0628?ֵՙúÈ@3Ž7y…À9¢¼ƒ©mÀ;ÉÞuk¼ç@ÇÌIo4Á@ñ·?œÎ?¹gj3%?¢ähÂ-®Ü?áïk'–Fÿ@­éa'ý¿Ýê¬[¾Ñ¿å=yþHÅ¿êr(a&W¿âՌY?6w¿çiš-=Oí¿å‰á`ÈWAGNfsrq3FGL J1736.4+0634MG1 J173624+0632?î`Bd»&P?Ÿ>è–dÇ?å…d•??ˆ™Dyû®?¢'x[(;??™&Æ:œ?ï6{Gb!?"-šZvEV?jB3¯q­?yºócêÔ?•õŠ!%†!?Ýá×í?éæ*Iáv÷?ªf0pXà?¥3+Çv
¤?"ˆ'ï@­?Ë朡}?¥Ž"ÎÓ?íŠd6X(ú?'ßTªæ_ü?'S
O±
x?xaYH²—?®°5ò¤éž?–eጬ4FGL J1736.9-3357¿ï¯šP½¿ñ];_QŸ/À9"#æÀ:cçl‹C–@'.TQ;@̧…ëfì?ÒyÜ>YØ?НkJѵj@i"a9×?ùîþ"n¿Ê±,Þ/u¹?çepûì¿à¡ÙÙû‰y¿ç.Â5D0¿ëcoÁXûD¿ïÞÜÏyOwAGNbcuTXS 1733-339?‰öên?ƒúµÛÞÓc? »+R3Šš?ž¤ý'ß
Ã?îéryD?¢¹Êš?c? ë0Ðý¤?£ãš{"Œx?´fØú·h?¶ºã]S†ô?ìw´qә9?¸m¬G78™?¸€)c}—r?˜{rHì?Ãa*¨ÃÕø?£YdûxÊ?è°)_W"?¦çqüՁB?Š­pM
Ý?s.|=þ'?±éŠ»?š¼­Gsj?íX·ÎçÝ?›|"´$OI4FGL J1738.0+8717?éÇ"A¯‰@;ô`RP/À:·9©MÀ<¯b³S@cÓù¼Äí@\Óû•74?À›íܼÙæ?¢ðæ t®l?âÍ*àÔ@´@Y‡2ŽÈ…¿î®kón!?ïý­_Ÿ!ï¿ç]à…ç5.¿ÜlOIoI¿äs¦¹Ù«¿â4¥>ŠFAGNbcu3FGL J1739.0+87166C B175708+871924?íNxò‹""?Т®$Ç1?QLM¢ÿ4¿?wKê>ÀÞ?µG5f‰?Йtüÿà?ïÎ:òQÍð?y–öñMýr?3ðDù›yì?EQbQ"=^?w£'‡P¬?x<WuH?h?ï)äG
 ?ƒtRù<õ?eIî{f"?SÛr=˜:›?˜9ZŒL?'žè‡2fï?ïýeÝa_Ü?&鷘5*?Îٌd{Á>öB‡H[éÒ?2—9Ãt'?&ZCå%9A4FGL J1738.0+0236¿¢o˜‹žü|@1€*ýڋÒÀ:n@÷À;ÙYæ%cg@´Þ'›¦@ÚÁLf
 ?ÍùdÅÒ\¯?¾$jÃmR"?åü§…ëg@#+©&?éVˁ¿ØÀPýôb¿ì¥Ž¿öЁ¿íÒÅ4R$?Ð웟-WQ¿¢HtñoÄAGNbcuPKS 1735+026?é9曝*?Á˜œ>uæ?«¸3¥Ç	¹?°i§íèÄÜ?Ä*X¨•C?¾<ZEcÕ?ìÏ7Z^\?¸L²eûÞ?'"£¾ã{?£âWÒÍY<?´ýž=ªÔ??²ÿ®wÈ?æèú?ùO?­¤ãì?¬žk1:½C?˜$ì¾p¤?Í4|3Ìçu?ªJB`Â3?ìd•´êiÚ?¨³ºòr×?h¡ŒÇoí?kNO¼0Á€?¼Eòq1Ì?¨J¥/Y4FGL J1738.2+4000¿êµUg:¡¼@>z'ÓºþÀ;ƒšSÓ½À<7‹öBçÜ@QÎCÅQ®@©ÚßµÝ?Œ)™pÙ¿µH@Ô±s?ò¿zÊÒ!@¦%‹ªÃŽ?ïÌi?‰­¾¿êúcÿÿå¿áŽá¿Î¼¿êqH'Š¿¦I`àÚ9·¿ïþâ=ø3-AGNbcuNVSS J173807+400312?דּd‡ul?ŽÈtîõ÷?_¤ºIW÷J?]â"Ie3?€Þ"÷¥å?Mm@ØÎ?îóþˆP¥Ç? ÷x‹•¯?mÝí~ð»Q?‰‡®'úè?ÄqF
/Ó?™ê•¦0Å?îiä8p€B?/÷*V®?s+Wäp'-?i(1"µù?¦üQ|ié·?°U ï/?íé&èAæ[?švþÖn"?[\#˼û?X•á2Š»?°J[Maž,?š'¦14FGL J1738.3+3228?í%êÙ¹Uˆ@<´›ùÆ*À;8Áo¡x‹À<}uôxãA@қ&·yÔ@Ÿ¾ÿ"°?Áø¹ò8¿»ˆÖ}АQ?øÅ̒ë)¯@ì|a$ˆ ¿êÓB1Ó¸¿ä̹ìö8¿étyN w¿Í{«ÝhüC¿ïÿÿ&¦³?ïÿûÞ]BüAGNfsrqMG2 J173841+3224?ïï[¹òá?aš"mà°?M~˜Û)?Q·7ánµS?S2<¿¬«?W">.oýU?ï‰eg'žz?àU&9?P¸î§ê¹?bé3·=A?‹–ƒdO?nðLð?îÓ4´ÅÅÃ?ŠD*uU‡?uË#­G¨R?rkÑ|j'Ü? P=ú®Ÿ?‡`먲·?ï—/`"«ó?|<yx`©Œ?WòõH–œ?R¬"‹é<¨?‡5É2Aì?z€L	+"Ü4FGL J1738.8+3822?çÌÇޝÒ@>ȸkùÀ;îQ{‡À<ö¦€1ê@!ØÚøºº?üóìFØ
?ÔrIÞñ<™?°å#/Úä?Ù[^€=ýç?ô'=ìs±?îÝ\á0¿ïE¸põ5¢?Ö ÎAAð¿é{S]u&¿œÊîÙŌD¿Ç-q}EÐðAGNbcuNVSS J173842+382104?î&¶rŠº?³™všu	?QÑe5ªWv?V«eB©ç
?­
­§ë?³&áK#?íBqN—ŽM?¶`ët>÷?†C,äڇ]?šfÊ2xÊ?³$î¨<¨?´U·F—x?íds¯	(?›À6n</?ûcfÅ̸?z+²×Cت?µ…oõ®ý5?šVgüÑ(®?éÝýdŸ?³žˆ²wÖÍ?u:¾¹<VÀ?u€»Å³{
?ÇÞ4wº	,?³ªÃh/ç¬4FGL J1738.8-3418¿îZlDn;i¿ùצ•*ŸÀ9O¡(TÀ:zòl™†N@ã""i·T@`ô¼ÕÞÄ?ÑÚ£Š´$?ѵ<O|@>EedÞ§@Õm¸?L¿æ"PA`ó`?ï%…€]˜¿é#Ê?SÒæ¿çb_I¿î'þ¢‡ÔË?©wìÎQ‡AGNbcuNVSS J173913-341749?µ""´}}?®2‰ÆÀ¤n?ÎvƒæÉð?Éè>¬?å¾æï½Õ?ŹqÖGÙ?¤(ÔêM?¤;" ?¸£¢
µ"?¸S')QŒ?ë¨þp¬?ºf`¡ Á"?½õ)Œ`Æí?™ú]U¸Â?ÈwÙؒõû?ªÎdì
ž˜?æ#dXO)£?¬;ö…ru?›Ù>~ËF?ƒ]ÒëÈ(?·ý›Lg¼"?¦t£1¶ÿV?ì!'¢|°q?§4÷³3N‹4FGL J1739.5+4955?²Üæ/w+@?·¸€®À92`8NûçÀ<CÄzî´@!;`©8@)æ~Nº?§ûîxn%Í?µ¸¡ÄË@
_`ûÃZ]@ã¤bËQM?ú+ª©¿á^Z(j'U¿ä¬…>õ!¿çêÿè­ÿ¿å•‡9᣿åE~Y¢2ÅAGNfsrq3FGL J1739.4+4955S4 1738+49?ïµ3ºá¼+?z¼àîÒ?JD"ÏP?WG¤'nà?Ñd5?xn¥Î¡Ç?ï´ÄÐÇ:t?zxÜQ?BȆ´ÛºÅ?SŠ8uS?¢Cbã§,?}´Ú5¢5?îöÞæb§?‡¹O÷öòO?xÿVA5}?q U¾U[?šäM­ædc?ƒ+7îÕÀç?ïéC8žß?Qd;¦ØE?CUz½ÉM?5]5"ȟ?açh±Ú¼?Mæᩃã4FGL J1740.0+4737?×íÈ^ÂÇÕ@?_Ãb(À:< Ÿ²¸OÀ<aë­b¤@¾éõ§Œv@$§š
\à?¼åúÆ/O?±."AS?õÔpšœÎØ@©Ì?ïÿÍ_ï©Ç¿æX}o—h¿ã1Ÿ_VQÆ¿Ùº-Ç©­¿ãQ@¾Œ¿æä&ó|AGNfsrq3FGL J1740.3+4736S4 1738+47?ïyÕ
X—¦?²hèOt]?Y²ŽÈÍç6?yÖä.ëAX?ŽTkÀY/?°Ö6n¬¹?ïžûÞß{é?"þþ7aþž?I@¡•Ð_?WÐXב ?†¬þ.Ãÿ†?ƒTæʐ®?ïÃ&yˆ?'¬.œt/?d'ŸìfØ?Nó¨ºÅVê?šWHk3Aó?ç i\{?ï%LQ~G?xØȘ¶,?{Ñ1!å
?_ϵl†60?""9ɇ½«?v€~¡µÀ¨4FGL J1740.5+5211¿àÁŸ2=r…@?ÂU:Ä÷ìÀ8'Û¼SØÅÀ<#ÞËÒÒ@Eãdú@œ¦Êı?[œ"?¡ñ=;í
?ü.x?'æ@¹'ÇÅüϿϵšðg¿ãõ"!	ºê¿ç?']<9¿æm7:ÿ°¿åWZà f¨¿ê¡7¦®AGNfsrq3FGL J1740.3+52114C +51.37?ïâÞ®[#?aÍ6"vF?<êZ"õ¡ï?5«ÎíNƒ?i"R^1à?]pÊO—7?ï¡'šß
?––'H¨õ?C0hò‰úI?Tçÿ­¾ˆ:?†‹˜Ê?–eËtþ®ê?ï*a>"!à?…Çs=<%?ik³4øÞÊ?Y
¸GlwŸ?—†aÈܧö?"é:{âwÅ?ïýšèË?' 'h?Á–Iƒ?¾1J L?-~K(*{?#ßüg—6å4FGL J1740.6+5346?îÙdý"@?Úuy(àÊÀ:WÑù\xÀ<zp§@Xâ»Ìtb@ÀàpÀ?»Æ.£ ?½…®À>•@ÀÄù™´r@oo.ah¿áDãß»¿æ\ÄÞÁ¿âVÂïÔ8Ò¿àîÚÞÞGI¿â	w­¶‡¿êÕC^#¡ÆAGNbll3FGL J1740.4+534787GB 173932.3+534742?ïðº¸4Š¸?R9˜Ã·?:"é²¥v:?4ZëY{Må?Wå•*A1W?O§q÷dfT?ï¯DpNñp?Yã{‰O×?=ëBC•8?Nz—îø;?ƒ?‡1‡?€M6ÒÏ?ïT…¹ŒÜ?x#ƒÏY2?büŽ­Ào.?Pý¢—ÖÙ?"ýsV‹?uòº<qs?8V?ó?q»‰&/æå?h茖4ÿ?S1Zþþl?†wÇJv?p¨Û`Ì4FGL J1741.1+7226¿íýO&"@?
¹pޏÀ;	³Ýè~À<ÂDK‰kN@:äƒøž@êp?ň.!Ña?¢¬Okx?Ü[Á|Œ˜?ùšw_²íþ?ìµæSҐ¿Ü¼ã`7"V¿æÃr ÜY¿äAß¾–ÿ¿áP2芘u¿ïÿX¥³ƒPAGNbllGB6 J1741+7224?îæQ=H-?"Û;ø¦?qó¥¬PéX?rO,i÷?ž¸õíBÀ
?'(V‰¸?î:ê 7N?£ðDçNx?|{ö"MÚ?ƒ#ъ..?¨ÁýAj?¡KÇø®2»?íŒÃ¹'†ö?"ÏD¹)£^?3• š¾?ÛzÓXø«?¯æß°ð¨?½ɔ…?í%™IRo?"j)xg0?œµ2¨Íqk?‡
›3¡«?¯KÒrNa?&é.‹éí4FGL J1741.2+5739¿Ø÷"ÁME@?븝jßÀ;ø¢t4À<­2.@ö睸0@eÄ÷1$?Á"ÑöØ9¿¨Í¼ì"ù?è›NÇ@
JML¹ìö¿Ø…o«‰†&¿è"Lá<P¿èbs'ƒ¨l¿à"NÿA"¿à*6¡Ó¿â÷,ò§QéAGNbllNVSS J174111+573812?ï×Þ6)—?nܐ²J?Lê‡È f,?B&‡01?ps"ò\'­?lE'X•ü©?ï±öOøÖO?€ÃKêC?><Ù~Ožñ?Qè}|?'…5×ï&?·¥6¾Q?ï5Xd4W?}µÁ¤®Ùj?cˆSÈÛ¶Å?Nµ<"ê€?–ãñú]þN?{é·µ—w?ﳶxÐÏ?jŠÄ¹õC?FVå^ÄL?8ú»õâ?Û¬óuà%?iÃ䜨M/4FGL J1741.5-3119?鏿åw'\¿à¾+IÀ9CUÚýçøÀ:Äz³ûD¯@È©¿±V@t6¸ù±1?ËϦ›à›·?àÜ{@" @¤˜"¡¸?ü(3/­AÂ?è<ÉIŠ¿è°«#.Ù¿ÐÄ?Êñ*z¿ásÇ­©¿ìzׁ܎Œ¿îpÍÝîÞAGNbcuNVSS J174126-312329?m¢"7÷ß?`…ƒ‰Ï̇?¶Uø=q?²šüp†?í¥ÁJZ?²¿§ÆÉox? ±¸ï.Ò??ÇÕ#ªF?¼ŸdÞÇ?¹®"²ë5i?ë`÷Õ40?¹×-UŚ?²Ë"–ùš?¶¶ƒÕU?Ñì¯jþ(ù?±ÈÇï±?ä°5סɰ?°Ÿ­IæUf?Ž—»É+èŸ?vå&%Û­F?À±Ç·Îœ?ª«+dªÄ?ëY/M-\·?¬Y™}v†4FGL J1741.8-2537¿ç;£u¡¨î@¢å€!ùOÀ8Ôê~ŽÀ:æ[{PÙ6@ &½´«î±@'ÞkZÂ?µqÞ>º$ÿ?Ûä'Z?ÜW!O Ñ@tKøÑãb?íø©)Y•ž?ëù>Dß-"¿ä΢o>¿ä8kì¸$Ÿ¿à½!Þ÷ò•¿äˆ×~×AGNbcu3FGL J1741.9-2539NVSS J174154-253743?ËMOÏ9²ò?¸yû…×?ª)êxÐGã?¨Ã•Î¬0å?çŠ
d¤ŽÆ?½rã
 'ƒ?ÜçóÕC	?ʨÉ~E?˜ ®3Â?¤o4¬X¸$?àË£ß͌?Éì§ãM…Ÿ?ÍrÀÆ$¶Ÿ?°=é
Üi?²¦9Ÿ$j?—¥œ 7.?æNˆ­bíÌ?°?ñe¾ñ?Õø–Â+O?°ð	'A?°;_ß[d:?—HÊèpò!?âüH£
ýÒ?±TU¦'¸44FGL J1741.9+2555?ïí²Ž:É]@9ý•1ã¨À;,PFipÝÀ<­^éšbí@½!ØAõï?ï0]€c½•?ø£Ðä¿?é¾ý×0ÓÝ?ût8Ùeb@-bŽÀx¿ê×ëC°Xù?ïÉxQ{¿å4µê28¿¡ý Ãô$ï¿ïÿú Âî'?ïÃk$;H«AGNbcuNVSS J174147+255443?î¼ÉXœöZ?®/
«Tb*?"À1ˆiÿ—?¨oLëgj?"¦£c÷5O?8T¯™*?íde±B?Äö#RYÃ?¦+åµ66?Ác*07?£Êz6¨"?§–î)a?éÝ{ŸŸÏ?§¯
þc?­1wåüÏ®?–]gXáB?Á?(LÓ?£)1'â{w?ïGòü±Z?ž)•á,?YšqÆzH?ƒ~‹¼Ã5?•tZŽÝm?šÖ\ÝKQÖ4FGL J1742.4-1518?Òèô
Œ
H@פ?åÉÀ9Àºª‹YeÀ;_Œ™¦@*ò03¤r@1ú´f¤?Ðç=¼h?݆T"A'@~€8Ÿ"@¥uT ?ïÿÉ仿⸗ÁREG¿æ×í\M¿íø < ¿à— /µÐ1¿îôú¬)AGNbcuPMN J1742-1517?Ç"ÝH=?¿à•¶2Kc? jJÄ*?›šPƒ2'?é1¶o†ï?À"èY}'*?Í¢Ä^Äu?Á¬c‡-A?Áe¾ìŠ&?¼"Y;´?ä=ßclY?Ãn‰Y7"?Ô¸ô#pÇ?¬¶JgÏ!?Å%©	œò?ªŠ–ºÚy?àZp[«à`?®žÕ2¨ë?Ñ	‰šÙÜ?ªünÌ¿Ú?¸
aO•È?¢YóýRP?äy‰9?®ôen1¿4FGL J1742.5+5944?ìFj­m@?Ⱦ
í(À:(1ø .À<˜Â^§U@';‡j—ù@RI^ãL?¶WfwÆ?›šà|¾'Õ?å‰Eû7@·º×Véq?îú¨Ü,¼¿åÒÑß^¿äø!å-¿ßÈh"M×ú¿äpƒڐۿäÍÝ·×AGNbll3FGL J1742.2+5947RGB J1742+597?ï¹1"ñÛ?rg<©"?UpÇ^?HlFÈ6N?}ëT—Ý`'?q$H"°+?ï£]{_aó?"}íyœ5?Lï†Q ™-?]ÄM­Z?…Y¨Ã
y"?'O/)«w"?îÚèB'N?†2<\‹ìï?pjÅv¡°"?[¤Þړð? D#)é†?"Nпԡ?ï_ 8ÄŃ?sïez;y?ÓcæXe¸?e
‡%Læº?ˆN?Û¢kÕ?mþ¦O¯?l4FGL J1743.9-1824¿êäò»ý@5JœÀ:%N1¼:®À;欇²çH@íwÜ°oŸ@Ýœ®÷Ð?Ð3rôb³?îhOt²Y"@èK èBt?÷1=ª…z(?î»ïÐð¿ç±aË×Ú¿ÔÂ܉r¡¿ëDjÞEE/¿ïÿßéà
¿êÖj€˜AAGNbcuPMN J1743-1828?•l¾
‡Ë€?~¯ÂXêà?â]ðíC´Ü?Ê[Ï;ó¶¥?ÙíRDÐ'?Ê5ËzC¶?›Ó
d?®˜EbI3?ærøóuÝ$?̘vçiA?Ñ\ÔHn?ÉA'¦©Ùg?½Dë"×Q?œ×³8¾?âgWüÆ?²œ/íX?Ôsö‹¥>)?¯•÷u"'j?e=•êýE?TWi?ë³öÚ«öö?¬Z,σ¿?ÀÛ.=§ð2?¬ëìsO:4FGL J1743.9+3747?î$5úÈD@<è˜_ö"À;g5¼zo2À<»-0º²ï@g³îY?ÿuÖ[æ?çéR©ðÿ²?Ø*HþÌy@?ógÄՇ†r@œ*M[}¿ïñ4 ›–t?ïýìo¡Î¿ß¸7^»ø¿àͶ!Ãg¿ïIűO˜Å?ˆ`NQû(AGNfsrqB3 1742+378?ïGF"–×?ŽÝê[øU?y"ùzˆ¦ò?vÍ?v­ô?µýNœ»_?Š-S¸º½è?ï7ŸTT™?ž& `£?dpAg3‰¿?|‡Ï÷íý?–~èŽû ?™1üÇ4Õq?ën¨GâÛn?¡J¶Íð?¨$ùÞs^Í?'øŠ+^öß?¸x@ѯu(?˜¾Q[rw?ïrØ4]Q?ƒ7šmõÄ?X2Ò¨r?b‹0Ôaø"?;Gç+-?'(" L4FGL J1744.0+1935?ïºß'³@7SÒǸÖÀ9rƒ\@sÀ<ÀÑìÇ>@¼ß7Þh¬?þ"à¿ÈØL?±'×
hcÂ?¢ûW¾q¯	?óÄÞ ²'/@‰Î³£?ïÿÕØå	¿ÂMæ<à[¿áìÙ|Þwð¿Õ³~G-»û¿â›õ>…÷¦¿×»s^"0AGNbll3FGL J1743.9+1934S3 1741+19?´$ ?ÐtR<Bo?MŠÑG7?CÌâ¥p?†7r…úäO?~<€dµ?ïcæ'Áe±?°y¾¢Q?a'ƒåQ4³?os®m!i\?'Pß+)"î?Œ£BmøHr?íîæ¼Ñ-?œX¸~Ð
?†cWµO"ø?wøΤôp
?´¤Óoƒô?™¹¤0Š‹?í^icm$?'ð(WÖÿç?šŒÀY[á^?'X@ËjÃì?¬Ø9==?ŒÝf%ü4FGL J1744.2-0353¿í5¡ä…"ï@*B®Ñ9CÀ9Í·'Ò$ûÀ;…}Ý{pº@ÕpK¯@meie?Öø]i?³ás¢äñÝ?î=Å}£ô@+NVÀ¿ÕpÔ^;Ÿ"¿ã
8bGõ¿è4Ž}å¿ä˜òü¿èÙïÊþ–¿ÂÒ°X¢AGNfsrq3FGL J1744.3-0353PKS 1741-03?é¤M¢Š?ÀJœmþ"?tۆØßï?l]Š]é2'?ÈÇ聆ž`?À+ùÞ?îcfSÑDI?¥BÖê—1?oÒ¶¢?yÕaÌ)‰?§ÙŠr?¤aƉK!?é™ý‰ô!?¯6W~8a'?™Üƒcd?ˆž""Iüi?ÈFvMP?¬ÚÆi	Ì?ê®´F!dˆ?£6†5YÖc?€Àæ!h?f‹fLùwç?Ä9-ÖLÈ?¢æ½kXæ4FGL J1744.4+1851?åm¿²CE@6ø/@_k À;\ŒñšÀ<™ªæÈ÷U@!v<_+߂?ü²7Pþ?ÏyïÓ»©?ªl…©?܌xžÍ5'@"`PÍ¢á?ïée߭п형";"+¿Ø¥þ—J4¿¸þ2ËYZ9¿çàm"R¿»ÉÐn
AGNbll1RXS J174420.1+185215?ï|Pü÷[?"%VÛö?@Ój}ä?2µ±"Ä2?ÞŽz?ƒíL;% ~?îýº¹@¿l?¡2ڔh?UÎlO86?c÷Åîêù?žëÂô'4? âð±ˆh
?íày{Z†g?"'uru£?p%f"^?_¡ÍÏ@?¯óÈ="5T?'Û8‹Û-¤?íu¦ä}?˜6Íø½«?jëbj¹"¤?auò"_Ÿƒ?³zµ†NK?—ô¥]"Š_4FGL J1744.6-5713¿äsÿðÕYÀ,\8Ÿƒ¾fÀ:
ٖߪöÀ<L|f'ëØ@ DÁ^.´s?þњw+?¼¯éè ?±tÏ	èâ?õ­`öºÜà@xM"µm?ïÿþÞ÷¿æ´ÇóI8X¿áX(`s¤¿ÕÙjj%š¿ßWÛßm׿ää2pLAGNbllPMN J1744-5715?ïëâ½z»?YÅígWÉ4?'=Wè?Uq@Gú?b¬'ÃÁ?X»'TWcž?ﱚ=I2^?‹*ÊvÅ?2¾´ÏS§Ä?PCVncd?ƒ{8Ë_?ŠX¥¥Ó˜õ?îòâcpž?†N$‡?eÆ_•§?d¤"ÉVÖ?žêóeùŠû?…ºÆþ€D'?îٗ?yt?';̲¹?f!ÃI¹¾?Püfó?F£?¡oÓÕ-?TªÌt;ô4FGL J1744.9-1727¿îFºÍ×õÜ@`\÷QÜÀ8ÁD× eÀ;… Äe@ ´©‰¦²\?þú¿"íÚ?ªŒŒk‰?'Ò1n?¬F?Øvd4¾@"8­ñjf?ïò6ci\¿Ü,ûáN2¿äJ¢»Jî¿×a¿â;˜ý'gv¿Å!("-¡¤AGNbcu3FGL J1744.9-17251RXS J174459.5-172640?Üés«ôŸ?ÃvW¢ÃŒ?sŠ›£Jn?o"‹Ž9Zþ?ád0ò¿¢?ÁM‰oã?ãtãÃ%)^?É5rë¢é?‹ÃÝ÷#H?ŸŒ
Q#K?Ø8‰üÈ?È×Ë%î?à^d
י8?´@U¶|ø?¡eÌi'ì*?Šë±ÉK#?Ý~W+Ð?³ƒ½Å9-ª?åÙxÛû+?±«úv{œ¨?¨ììu7?'Êaù™ë?ÑI&¶[?°m&'"®4FGL J1745.1+4731?Ù‰uÏ@>ƒô˜Ã°ÄÀ;T֍?ïÀ<¯l‹C•@º
.k?ýñ%Vѝí?âN.r±M?ÖÄ2I~?ù[4Ú@vkÿØgá?žÖ=
ýn«?ïÿnw¬à¿äY®'3÷S¿Ùv™ºPÉF¿é¢·…<ëC¿ïÿð ¼x—AGNbcu3FGL J1745.4+4721NVSS J174501+473247?ïbD+{Ë?Œû MA$Å?»ó†?…¬óŽVá?…³$Ú|ñ?€¸·ø?ï+æÏý?'+û±z?V'E´»?pÕdËïxÚ?bݺµi6?Œÿ=Á=æ??íü{`é?•ƒ"Ré׍?^ök×´?€¡OÏâ»T?®Hz¯
ù'?'í:õâ»?ï9·á~Ô«?']Ñh(=?dBç®É¸?d‡'ƒO°Ú?–@¦ÚL3ˆ?wMNŽ÷ó4FGL J1745.4-0753?è¹Cá‰Ð×@%£ôË—¦À8ØûíKÈUÀ;ktà |@Ðrá@‰å\ËO?ªŠq¼
•r?†:¯1ƒ?Üùº@®@øìÂ
¦ø?îÃpbhªä?á¨Ü,¼!¿ß¢Ž4ቿâòMà]£I¿áP©ôg¿Î'ÕDÀyWAGNbll3FGL J1745.4-0754TXS 1742-078?ãÔ9y?ÃáöåyÚ?H·FX¨?†®ˆxŽJ¼?Øõ° ÌŠ?Đ•ð!ó?éììÇÌv?ÄãõÊr?'u\óOÛ"?¥×­è+?Æè®vÒÇ?Ã{Í$¸9±?á+3ŒÉ¿?´mqïKɚ?¤ÓÄޙÈ+?Žà¦¨Cù?Û!c3~?³±®üg¶î?ç»úÕµXÐ?¯éyÔTµL?¸<ÂU4@?¥WŽûµ?ø?Äñ³šŸ?¤Ý±qzÌ4FGL J1745.6+3950¿ígO¼Î@=Â!yÀ:ôÿ—$tÀ<¢þ~ö€$@Ú%Oð®@ËÛjõA?ÀTUØ#Âþ¿§ñi~º?é{~h?ý‰J°Rn¿ß?ÒéF€¿æ›#Â|粿àÉÍ©kžµ¿æ[Ù_'F—¿ÔöÜÀµ½¿Øˆ]|\òÊAGNbll3FGL J1745.7+3952B2 1743+39C?îJŠÝG?§¥Mà Ã?}2ˆII4?{G{>ê[?§»¡ÒP?¥!@Þn?îži<5µ? –1­ì&I?p¦ˆ\µ>?~Š‰7ôÝ?¤•ð¦¨?Ø2²Qþ?í¡ƒƒ¾Q«?"2Å4ç9?yûøXÕ½?pFHUЕ?°Ä¤cWò?':묥¦/?í'}¸¥?™JgVéL^?}è¢vd"à?sd@Q€ ‡?µ$áêԎª?™">U"ÕÂ4FGL J1746.8-5235?î€
I¸ŽÀ(v³™õßìÀ9Ågqÿ ÝÀ;ª'°H1È@^+?ô·¢@VF]²c?½—Ù%Ê ?Ï¡G"~Z#@ÔnYyîÙ@Œ>gCÜ?îÞé?Mô¿á]ʶr¿åî€F}¿æI'*K'¿î…ýÉÄÛ¿ïýß1S_AGNbcuPMN J1747-5236?ï:´0(6?…%sáØb?"]ìä²÷?µ‹†?o¯ÔDý
?hBŸrz²¤?ïjôT?Ÿ"g ™?JNy–IqÍ?gV•¤S?'Ï°‹Ñk?žbl´Ñ¼?êuíü$š•?«þ¬4ü‹ó?²ATnB€? .±xdN?ºANÊlèÝ?¢ ¨RX?;3?'gU½\«Û?vƒ$Š3Ùg?i)qfRÖ?£÷7¶¦S€?'A¼í4FGL J1747.1-5453¿Æ™0ŽÏLjÀ*Àaé)#æÀ:=ÀÙyƒzÀ<	¶Å#‹ @Ä>tÎ@²ÔüF7?½g'¬lZ¿ãKX1ß?Î]èHSV@'ß–S"?ïøæ0K!g¿äFÏAò׿èèmÀÍ»¿âMrU€¿ä…áUðÍ¿éï¯OäCâAGNbcuPMN J1747-5450?ïáß¾—ƒ½?`Ñâk˜8Ü?@Rò&l?2ƒŒÔ¹_?jl«õ9…?_$|o?ï¶Ä%,á,?"Z.:=-?+Æ[´ñÜß?>6`¸ø?ßÝEóí¸?ƒÝ)_Õâ¬?îÞÙ±†N?‹T¦þƒÚù?nÅd•ÍñU?aǬ÷⬸? 1¬Š¼?‰Bïv úL?ï>:e˜ú?unBñ=w?XZw'Ee?CL¸v@ØM?–¶ÑAºl`?tÿù"#úÉ4FGL J1747.2+4937?Уløb
"@>tºËB‰À;wNÍÃlÒÀ<Ø[¶	;é@!
ì‹?ý²X''†?ËsyŸSAñ? »`=ØS?Տ¤ÐÚN@Ai'^è¿ïÿþÐñ?ïÿ±üfîL¿å5=߉'æ¿Ö3)"89,¿Ùð«C"¢¿Úœå¯ºAGNbllRX J1747.0+4938?ï×ï`ô?qk²"Íån?.Àâ»tQ?)íiIg?s€_óãc?q"Á–‹é…?ïÀäôU?€â–ÖƎ?.ɯ8Wú¶?@)_®H?~ÿÀ{ÃP?<	ìÃ)%?îlx¾?ìW'™˜?hñûºj?\}$Eål?§¯(»'ؾ?Œ²>ÐKæð?ïŠr"Y.&?sk÷ô"V?R›n£æv¹?Edَπ¨?‹	•7¨?syò¯¼OR4FGL J1747.6-5308?ï·-s€«6À)/ñù¬ÿ¨À:oëBÙÏÀ;ö¶
¨@WS(q
^@~=½Ð°‡?Ä!_÷«¿ˆ†ê%´V?Ãì­è±î@µ›[慱¿í¸®6Ý?ï\£¥¦î¿ç{]U¹¿é6çRŠ¿ÖæÙ¾L×I¿î•¼Ê÷	·AGNbcuPMN J1747-5310?ïÛi=î2œ?‡7eõÃ?FÚ^ìïü?Wù-Ž
?nà*VÉgñ?"vAù'‰?ï¸ë£ð/Î?‰Ý ´™?'ļüª?AÔu—$Ø?gó‰{?ˆžbÊý?ìQä"?¢º~-fœ
?‡aI/á®?z«#·ïé}?¹	Méܦ?¡'#‡csh?îŸ-Ui×(?‹öå:?[—íV/b?Rø†›Ë?¥0k>®ƒè?Š§5ØÕ¿;4FGL J1747.9+4704¿£µýE™õ@=ù'ÙýÀ;VTÊ\°À<À¿\¢˜@¯d'`—ð@é?^º z?Òu{{vn?ã–]O@	uü wnÌ?ÿ¼–ž½p?ïçÝ>´ñ¿Õ±¥^ɹó¿áÊá:B.¿é™+€À…¿áà‡_rV¿çÈQY•AGNbllB3 1746+470?çvèe÷F?¿bÅ%Mð?¸Ø*â0…?´Lë*
¹??ŸIZ0r¦?¸âv[OÎ?ç"fïƀ{?Åæ¼eñÏ?ÁŽÃ4žK?ÁõÍÌñ?À¡GàÊ?²'e7Áõõ?çBø©ãaV?«s—©Ñ.?¾fGlƒ?¢{ü–&I"?ÃÀùÍlÄf?¡¥JãY9?å(jìÑCz?­Õföf­?ƒѦv]c?«qÂ2Ó?Èڂ¦D"´?£¨ÈXÔîf4FGL J1748.0+3403¿íÌ_àÌo@@;-'d2‹À9ä3|‡À<h&£Ø·½@G¨Daª@Öé5¹q?»š¦c'?»'3`)¶]?ûÿ,ëñUB@ã¸cß"¿¦¦²Ü¶¤Â¿æƒ"Ó†û1¿à«Áïùø¿ãs[ýVØT¿ë¬»Ií‰Ü¿áË¡>(¯¢AGNfsrq3FGL J1748.0+3405MG2 J174803+3403?îĈÜðY?¯M³µX®?sí€ûuhÛ?ŒÌFÈ8?¡9¢MV?§Ïs¿^ó?"Dûz?"¾ÝØ«N;?PGÔ. ÷9?anCºÜX}?‡Í¤hí›?'—ö×ðÏ?î_‡]Öp?"¦oH+Âd?sð7ÿ(?‰Ò¢¡Ïú?¢*Žµæ?Šl\xD?ï}QO$uz?s¾žy'6È?oŸ+îe½ ?Vøîû7²…?ˆÃá;I1ý?pÄ
´ "ø4FGL J1748.1+2702¿¢‰=AY/ª@9‹¬q³À:Ð	sFHºÀ<~Êl <@"êƒÁëó@­[î=`?¿ûòTEÒr¿¥QÑìqX?çÛBEõ­—@F´\"~Ϳ蝘—;ˆ¿ãƒ¤?9ü¦¿è–Òª\_|¿â'¬¸ZO¿×™ŒÃó4k¿àÓ¸^€¾×AGNbcu3FGL J1748.0+270187GB 174618.6+270457?ïëÅÄó?{l¿A13?S¦®­ªÃ?I>XÌH_Â?†8¹I€Ø?z5hÔ$#×?ïªU.ÈzH?€õÓ8N¯?9•e±Ÿ?GÈ!o±"?"¡ãÙ6@f?€BÝ£–«?îú'íhë?…Išp	?e¼Z×Cµ~?U
Æ6n.|?ö÷ú%ô?"
âh)?ï_5²hå|?ynö$LÞ?OÙ£dŒÔý?Bô·ÃÃÛ9?"|—¾éÚ?y\nŠ4FGL J1748.5-0854?×^ÞutSí@#O27Š°ÉÀ:…#\%šÄÀ;ݐZU¶ì@!Ÿ¦HÈF@—:*?ÃIƒ—#ȇ¿ŸŽr@†¥C?à‡ˆàcØm@^ô¶uÈY?ï"ùV˜"	¿æÐC¿dT¿ë4tF"ú¿Ó§;cƒ¾¿ãºua«ì'?Å/D%ɾ%AGNbcuNVSS J174838-085435?ÓA
Xœ"?Â;‰¨¸š?smyŠ½£µ?k^'¯‡m?æ8Ÿàà6o?ÂYU\f|?Ö½ïèÀ¯¥?Æç9uf»Ä?ˆ.N†ì|?"²9¨÷éü?ä@Nуö=?Æà%örwØ?ä§#¡Eû?°áiÂ?™Î@ew?'˜CÄ©•?Õ×9o™?®íÒôÀç?⃐~«™?³ñ6cdÖÁ?,[yé­j?"ˆ`;ÊôÅ?ÙöK[ø?´F9±ÌÔ4FGL J1748.6+7005?ïÿÏ(FÆ
@>¶–¢nTqÀ7×m̌5À;s;BÌ-k@ðˎkß?ÿ>(	3…i?–PÕZîu?¨Œã¨±d'@'
¹t*@-…Æ}þ¿•nZ·Â¶¿ÚëèÜLòw¿áaÚ«¿ÝóÂo{¸Þ¿ãO¡ÓÏË¿âäî—!ðAGNbll3FGL J1748.6+7005S4 1749+70?ïë`N—Áª?XÏØBðéÉ?.]qÅbÈ?'I÷8Ž´E?b¹ÚKè4ž?WùêþSú?ïƒ@ Öáp?gAÕP?PÛ_³"Üû?`ƒeSHâ%?kÓãH?ŽjõÒB™?ï?¢h"[?"ÄU
	uà?w'ˆÎþsò?užz$>Ü1?''P»¾÷"?€ëc©ú?ïìǐ%ä?R®þ©€m?0Ñã½ÞÈ?#ìÏC¢&?a/î3b`û?QÁdá ªZ4FGL J1749.0-2327?×8§9t@­¯ÑƒÀ9"¸'ú
À:©"ðÅÐY@÷i¼‡/_@KUhè!?Û¬kBïó?à›q«>Ì@GŠLáZ@ñ҆õýô?îíN·ó÷´¿à*èÁŸòú¿ëÝõéüˆ|¿îç}R;6¿Ð6'Τ=b¿âGß½•LAGNbcuNVSS J174940-232619?Êû\Ċ?À²êWU³/?Êߒ6͌õ?Ŭ€à;?âÁܱµk¡?Ê~kH?Åár^Œ5ß?Åÿ¤²½ZC?Å¥ïµßæ'?Å*sýï3?å'zäøä?˒.Ì2p?Èë%õ½?¨8ÁÙ…?ÊKߎ
Ê<?²Þ'À{o?ã2 Òÿ0?´1<Ö.óÇ?°Ÿ–XƒÉ?šƒvÍ}?²1uÏ׳?­ß–Ú?ë¥Þzô¦#?°J',Q‹4FGL J1749.0+4321?ëÜoxo
»@=&éÝ~˸À9:ªö¹/aÀ</ë/³L@j©t@lŠ½]Ä?¨–ºÒ܏?¡§¯†ëÂ?õ꾅m@"ý™É?O?ʞΌÀmC¿â4¤ý¥Ý ¿â‰ôafL¿à"IÁj"¿ã%"R¿à–[@î\¿AGNbll3FGL J1749.1+4322B3 1747+433?ïÕÑæ_?hŒ:ÌÉx	?@A›&'wÁ?3ÔT{›?sH(9a'?g¤ŽPJH²?ï™D¨p?†'+|G5?M=²êE?b%§l.¾x?‡Û(,ØÊ?"¾p2‰?ï@÷v$ê?{'¨'ÄcJ?e¦Êúuhe?OñÈÏìá¹?•,7Ü»?zÊ°8»?ï‹ä>I?s%ä~؁?r>¡\q
?]{0ÒüºŒ?"¶0¿ƒ^?lËÕç=•4FGL J1751.5+0938¿îyv¹oÎ@1¦»#WÀ7ÃãiÇC÷À;PáK	Î@ ‰ôµôï@'òeÊ?šã[üÍgõ?¹^Þ¡zRp@;'—•@F]	pl¿Ç'*t¿ÜmùÞýQ¿ãØÊfÀÿ9¿ãçހÔPпçL¢Ûa»¿èMÄC'OHAGNbll3FGL J1751.5+0939OT 081?ï¯KK¢?zp=ÔfU?Gގnvñ]?C?åíøTs?'¯OFTèp?y¤g´Vû…?ï`t5üª¶?"kþVÁç?b¸ºr'6˜?r»ŸŽÀÛ?'šaò%Â=?"—™w'f?ï'.Oc¥@?Œ/ž½ËÃA?›™ˆ?#
͊›°?'Œ'ž'I?"@"ü=š?ï¬G€4¯™?r{Òã…ß?Qv'<-tþ?FVó	!ÅÀ?'¿MËNj÷?q'e9Æ2"4FGL J1751.6+2921¿ÚO=æÛí@9†¹ÃÀ9øzYbqåÀ<÷­K'F@Ÿ6²Á@™WÚ²h?¾ólɬÜÂ?À½oø
",?þ7Ó
ÔoX@3Žk¾"?åÞ¥µ%ç¿â"Px¿è=AÞËÓ¿çþ~pHg¿ë>¥Œìâí¿ïù‡ÀÔ AGNbcuMG2 J175143+2921?ïà'|íqÄ?e"ÚG??XÙ.a'––?U,݌‹Ž?cëáúp'?_±DۓÂr?﻾´û>¿?õ$}áº-??ÍGã7?SÆUÈSd}?€è…7a?}˜Ê[ª?îÿƒÜ3?"šN
—¡F?t°¹¡?`Ÿœ›îÒû?šÞØ_'1b?'w.ûOY?ï½°'Œ?fšÇÎÝô?Vٟ½ÑÏd?C"aZ+J?{q—HwÆñ?eH>£4FGL J1751.6-1750¿æ®†f@?éúÚýÀ9¤±ÓLBÏÀ;t<"¸@ ,šä"@¦ÐNaŒã?¾&—Ÿ-¾? […â­‰¼?ål"¹™@׏SD ™¿ïƀW~A?ï÷a–5¿åZWBÖ>¿ä
º}¿ÉY¿â"ö¥
k#¿×Ïî,ëñAGNbcuNVSS J175120-175112?ÜcvEúÍÃ?ÁÑÂ{·(ÿ?•¡'ÍUt?'"–êí]?á!;žšvt?Âç¦^H?àq¨^ðÕ?ÅN#A[l?ŠT!žˆ>?D»0-§?ÞK?¢MÞD?ÅÝ,¹J
?Ø6†šJ–?±Ò{_œÑw?¬\«éd²?DZg'?âæè²?±,a¥mû?âÜUÍ5rç?«U.?£|61 ¯ù?‹¿Gíše/?××͟a3?ªîñ§"—4FGL J1752.1+4531¿ïë薁â@=Îg×®À;%3BEÀ<†#mÃQú@Çkcü@¨> N¿?ËÀ#8?²šð €Wm?ä^¯¨Ï˜@ø&¼x{?ïþ°_-âç¿Ì7ªçݑ¿ëênió9¿Üc—¿yÓ¿ïh¿ëxá=G3AGNbcuB3 1751+455A?ïŒø£‹Ñ?ˆ/›ãË?oÄãU&?qû܋N¼?…Ð,61?'Û"AÀ©?î=öŽÜ?£Iõ¤ ¿Ï?n×VAÏ?ƒc·ï?¨2Ó÷I§? c4ƒŽ¢z?ì™_2÷íR?›i^à?•ôñ6"šÐ?"»[ËZ?µ·Ê›nÂ?—À\×T?ì¸óTý¢ä?˜ƒa–ù(±?¡Šh‰lJ?‹jcD8u?±s1Ž²¼?"V¡"c4FGL J1752.2-3002¿³—áðM¿üøÉZQ….À9]ʊÓ-9À:""д¸Ú@f­éê*@RaœÓ
?ҋ$÷0M¦?Ô½ÝüJô?ÿ€|¬ùÈ®@LH6z?¿_&¿ë¢AsgÖ©¿ç¾BuE|¿êY`úÛ4¿ïís 3*?ïH™"º]AGNbcuNVSS J175230-300107?ål;•Ñ4?ǺGªXÈ?»>:Þw<?¸'Š;^¦?̯ô9¸"?ÃvÐôžs¨?¶4£»'Ä?· -<?¥~~Sµ?«_Åî¬xÅ?ëá•æO»Û?¹Ô½º½Š7?ȘÙNtïÚ?¦Q©çT«¹?ǹš×ý'?§ú·Â®c?ä›E¬Ä¨?­D£ñ"7?˜VÆÖ.‹s?"¬;AÅÖ?´ âÿr‡ï?©dØm?ì¹-i`:¦?ªÝ—oC84FGL J1752.6-1010¿ÎË÷¯úY@ K›ˆ‡"ŸÀ9Íj'E'À;rèn@P(Ð	˜@C@ˆÊ>?Îľ ¹?Ú &5j@Ž"mR?ÿ¨]—4åe¿æ½8:1
?îß®áÕG›¿áÙaÏ©¿é…V`߾¿äõ³;+¿ß«©f–7AGNbcuMRC 1749-101?¦ö3ó:Ð?
Äûpî?¨U¶cm%?¨edèJ–¿?íAi™ú?¯ÄjfFiT?ԍª¹Ð^?Èh²¶є?Ññ1±Ÿ?Æ'û9'õ?ف@£§Ž?ÈÎÐWee,?Ð2êŠEÇ?§A;<×›?ÃH¸Ä#£Ö?£/*º¼éP?ã\‰Ô3…?«€÷Q7å†?Òɯ1îë?¤d^%Åz?ÄSϳT¡"?¥{¹Šø?á†4z3b1?ª–cºÖ˳4FGL J1753.3-3325?Úû|Ë`DÀ
ÐãF¶žÀ9¡Åè¬ý$À;–÷z€Ï@F³ÓÃt@uêgèG?ā¨÷…ˆ?âç@Áf<@w–¿Ê…Ë?ëX{-a¦Ó¿äBxùæá?ïøkç¿à	'Ë û"¿çM}™ù¿ïDÀ
¡©?ν{¶"¶ÞAGNbcu3FGL J1754.0-3321NVSS J175308-332637?mÜÏÜØ?h'p*ë'?ê9RMŒé?Án°ñ곜?Ƥ‹z­Œé?ÁO`¤â»?\UÑñ?—I—ûZø?å"Åéz[R?Ë(+oœ`?Óû'"–ÚÍ?ÊOµÎ^Ì??¦h€3·Xê?ŠbwCª?äõ'ºC *?²uŽd§ÈŽ?ÓH …Ԑ?±%ÁøÆ>?'OÍWB]Ý?hM ¡
ÿØ?évXôå'?¬Äß´hÎ?É¢º¸D?¬2:·º54FGL J1753.6-5014¿ïH¯p4_GÀ(3¿ÂÀ9q¾íæøÈÀ;ÈLáZ"‹@™Ìs™@:œ£9V?·íÍ9Ú?лWYƒ)@ó ÔƖ@@Ÿ7=Xü?ïôT›bÇu¿áÔX<×ø¿æëªÞe{…¿é
áSíh¿î?S‹˜¿ïþ7=ƒï
AGNbcu3FGL J1753.5-5010PMN J1753-5015?îÀªÃp?œza®8¿¹?"Çßþ@?SO"Ø <?"6§^Ǔþ?"'ºJyë?ïr­Çñ
ˆ?™¿õ¿Ï#á?RȒ2ɱN?cÝ\¾G©ý?}½Þ±´?˜Û\&]"ò?ééÝ´±ƒQ?¬¿0Û²P±?·"
ó­/¹?£"Ÿ)¥1?¹fƵ¾?¡B1W?î£K'ã¹ú?Œ–ԁ(h?{¼¾Æpk6?m$•óh?¢S®øöRõ?‰Uj©*4FGL J1753.7+2847¿çþÀ묌@8tH@árÀ:écO͞À<SuDO»)@'°
ú> @Ü@Þ¡,?ÍÎ#äᖈ?ÁPý¢}C?ô'À®9@¾·ëêl¿ï¨"¾é_U?í4nfåè'¿æÍöÎ(Ÿ¿ÜI¹à<¿å'¶þ.o¿ïÿnªØ†>AGNfsrqB2 1751+28?ïªX$Ô
?|rGØ$?`»{dk–F?]ã!:!…?;ñãX?xÔÂd.?ï"Ïʍµ?†w="Dq?JÞ ¤VÍ?WN×ÖxÐ?‰^+[>
y?…¹*Ý?î—fƒb¼Š?Œ¼­ÊÅJ?u¾­Šk,?oî:us?£Ñ†Ô
?‰l3UŒãN?îáuÀÛ?Â?ƒ|/¦[H?s4¡…°'?`Ó\˜l?ŸƒWž?'¯G}4FGL J1754.2+3212?Ø"Ÿíƒ@9hÇ\Jƒ²À8|'¿bÀ;'=mHØ·@üµ‡‹Ð?û÷BÖ>f?¤v3ãÝ4¤?ºüYxûê@'V†''@°Ž'ºR?èÄHÏ|ªv¿ÜØP÷¬¿ÖL˜_¿ÜšäN¿ääúœ>¿à#Ü~¸AGNbll3FGL J1754.1+3212RX J1754.1+3212?ïâÌHöïû?a"Žæ"óù?7á?1,À-Å7J?j7‡'ŽBù?`ÔUŸ÷êw?ïŽ2 üêT?ûwsö?PvƏ4è?`oOé~ð?Šdžþ3"#?&ͨx×j?îú¤{F,?'¯ëÙ¦÷Ž?"gÝôöf?†R\»yn®?–{Üv7K?‡"9bG6‹?ï©Î/—Û7?q¬âÔ¬þ?E6I'"ôô?6a™7ûo?"9àâÇ?qac/O§Ô4FGL J1754.5-6425¿çwck+ÙÀ2yhÍJ¡À:÷È#àÀ<:©€—j@bÕ~w)W@B:73s?ºŽ4`¯Ã'?ºOM:ö?þ,—£TY@›ºø9;¿Õ6³t¿àTΎmìm¿æ²2í"ò¿æ/
¯†k¿ç¾;]e¿ä1RB˜AGNbll3FGL J1754.3-6424PMN J1754-6423?í}¾Mo×?§MåGc7X?w<3ôP¿°?nW#ŠÍjs?²žJX?uE?¦¦_|~p?î s$+y¼?¢Cû98ææ?vÞ¥ºú±?AÓúâè?£ùé-?ŸuSò·†?íT»*¥ä³?žSåÝ=€?ˆq|m;ô²?z*.‰À%?²K÷)[Ô?š¥&<b…?í.«ÆÄ?'š[ÞED´?"³yϲ	7?x}9Îÿ?²R µG"?'f²WëEÙ4FGL J1754.7+3444¿æÅx'®‹@:
~À¨À:ÉÕTZËÀ<YT¹•¸@Q]f¸pÊ@Ð_ÿD^?Éþ¬˜ÏÅ%?Öèè÷¥¾k@×èÚI@¨þoÝ­?È+Ê^2K¿Îy™ßd©ù¿æ¬¾´ .¿ëOÀ²0¿ð?ìçìãÉWAGNbcuMG2 J175448+3442?E9QC?…‹iœþt?q[¥S¦Ã?xüŽÉȌ?}D¸±Y–?|ðÎCË¿?îôÀ¨Ãù?£$ñ~ñBû?tîõQÂï?ˆ?—Oøl?œ,.övÄÛ?PëúÎAÿ?ëú"<•?¡
ºªK<?¤ÿ¦ÓZ?±+¿˜+[?¶×C"‹¬?™è¥¯"´Ò?ïOÚ3ŸòN?)ÓÕ+L&?hN1•Ÿ?Y7´Õ¾Cß?'úókƒN?‹:µm—4FGL J1756.3+5522¿Íׂ©Ž@=¶ê šª;À:€~?¡À<e–È.›@ a®.ß<?ü6À5¯å?¶oçnŽ¨û?±3nÂUz†?ûgÿÚ$@æ~ÜÿÊÑ¿ÉîRCÙk¿ä s"6‹­¿ã€í0£?¿Á5µÙì¿ßÖ÷¿àÏ>šõ9AGNbll3FGL J1756.3+5523RX J1756.1+5522?ïÅJ7†I"?'^DyÜ?EÜï½?Q[÷òÄê?zŸF[>V?U?ïš#ÌÙ¶Á?†åZš½?HõŽÿ»ùÎ?U[`ŸÃ?‡ç³Ù–:?"¼§7÷&?ïÊèM·?'çÁdÄC¨?bþõø$ʏ?Oºy°lJ?š†Ä@'¯ý?Ü‹Â&{?îɜç7?3ÔÓÁÂ?uTä(1?a_Œ«Â§v? »•g†,?ðîzëe¸4FGL J1756.6+1553¿ê;"´Ñ.@3PÅë1<À;ۉ(2NÀ<†@Š3Ë	@!M•¨H^@&IlÊ.?ßËƽi,"?î'­ù¢î­@ñ'À8iÔ@i@e˶Í?ïþ@Bo	¿ïü­?"¾¹?ï‹4|¿·^koe¿ääc1Ù¿æ<ÞÏ®©AGNfsrqPKS 1754+159?뫛5â?¹õÕ@C:??';Ò´Eޛ?"½HKP?¾2q?x,?¸´"Xìtb?ãÏÔ2WÒ¬?ÐÊ;æ/Ȟ?Í`6)?Ïó¤?é>?õO'&?À!Γ§´?ëNà–­m?¥/þ–ÑJ? e¦ÆJZ5?'MJ2õ?¿šµ˜%g"?¢ŒÜMêR?Ùò·"\¡œ?Àž·IøBi?Ê;º;i?Á¾*þ‰—–?ØïÁ€…©Ý?ªXâ¼ê4FGL J1756.9+1531¿îÇú˜7ñ@2æãæÄŗÀ:ðHG—nFÀ<b.bT@»ÃZ]C¨?þ³(fP–ñ?Ôào Ê$ý?Ñ¥7<WI=?ÿZÐeށ*@lÏ,M'?ïn+÷Տ?íû.t‡'Y¿ìp2˜Á?º °º›í¿ïÿÖ_Æ	?ïú2–UA{AGNbcu3FGL J1757.1+153387GB 175437.6+153548?ïi—- )"?ØVá¹Ø?p~KUk÷¡?r1;'ƒ+‡?[
?Ÿ‡?ŽÆF¥-Òð?íðµ–Î(?±ÉÛÖ¿(ì?‹]è¸W½·? HZ¢R+?ª4ˆ}.?«;5Í}š¿?ëY~ªr¸'?¡Ö`úV}K?¡à00e?Ž8¢¹Ê1Þ?¼Cò©R7Ë?ž `ßaÏ?ì|h1ÂcÞ?¦dÍUrÚ<?—°{ÝX&\?"'×n1?¶0Ÿz–×t?£êفtøG4FGL J1757.0+7032?ì·L¥þŠh@=ù…H©¼ýÀ;‹y¢ƒÀ<©ô§Ý);@!· ê±9H?ûI>‡û¤?ɳû*-P?¸4tѹ?ðK'ëk:@‰LC$—å¿ïêKÎ4«Ù¿ï']Àz"?︶•Râü¿Ø˜±ý""¿Ý/<Ùz/¿ÖAW›:ÙAGNbll3FGL J1756.9+7032MS 1757.7+7034?ïÌgÄÅwn?Š¼Íræ
?(¯y.+±??ȯ²ž˜!?y¡Õ
ØI?‰2;¬zzÖ?ïv"ȼ'?•í$?¬	–?I"Tø	`?^–e<ùª?`ä@­a ?•#äeº¦,?íû‹ã¢à}?—óöž¸/%?cryß+¹v?TÚЮà™j?¯'ß<–?—–?´7ãc?[sˆ?…æÚkY?OGI¶+u?M:†P¸²É?œrP(ƒÝ'?…†/"ãáæ4FGL J1758.2+6532?âi ç…y–@=ý)WÉÀ;K³ò
s÷À<¿ÇòrxÃ@ûX4õU,@åùÄ|œ?ՑBq>²?Ú*–ÁøÞN?ëáÉ^-\Ú@¬Ô=Y|É¿ìA#`Ø2¿Ó‹ûKeY ¿ä×	 åþ¢¿æjK˜"Ƥ¿éK§ž?¿Ïž¹(«õAGNbcu3FGL J1757.4+65367C 1757+6536?éPªy\e½?½ÆVð¢W?¡_UënHô?™©KÚó
?Æe€Ÿ²ÖÌ?»¡Áè(¡Î?îZ¦ÐÙ?¨C%xl.?€æÖïJ¶%?Tô4E?¦ÝDÁ"?£Te×)?ê1ÇM.ât?¤âËT)þ?®!C!Õ??" i'¤|?¿a$žhÁ? 9£òŠ?îäø¸÷ð°?ù_œ×þ?}£(>œ©7?hDX̓°s?›øÑZ¿£?ï…ØP>4FGL J1758.3+1429¿êôãaJå@2.ä¬yÀ:'¶ªK˜…À<>­j0öB@®­€VQ›@ÍæÝð
¿?ʞÌßAC—?ÊÑJµÛČ@t¡'Œ_@dlH¨W?ïOÇão?ïþ"û¥'l¿âݸ½vB§¿ákßj‰6¿âøÀ$óª¿ïü;±îAGNbcu87GB 175603.3+143022?ë…6õ1'?´§ác¤˜œ?±¸ÄžôÍË?°d›d®$?²‹a¦*?¦—Pþ¨x²?ìÝ«ô.t?²¤[
žl?™́«^1?¥fªÅŠ@d?²·/?ó´à?©fì´'Š?êþäS`?¥mDoœö?¥£ÿCdæ?"'¼gû‡?½ƒ
åÅZ…?Ç€¢4}?èórÔÏøH?§B	rlRè?²* ß3*?á«Ùƒùh?Ã$=&‰á?¡™":›4FGL J1758.3-3028?ïÛΘE À	VDÿäQÀ9‡¨ÖMÀ;$Y'¹'m@я‡G¥@,&Mq£?»J}ãÁÂ?»&@Üi"@¦¿òÉ·@λÁÎj¿Ú—"š|©?ïòZ€T#C¿âž/`?Û¸¿ä¿ó5bB¿ç(§ß, È¿áå˜îxïAGNbcuAT20G J175822-302916?æÿ4EeYý?À!Gž÷¥?ŒÐhÖž?ŽAÇ­´g?Ñ."{‰?¿©i"¡ƒ?â°Ä˜ü|§?ÈÃf²í`?ƒ7õ(–Œ?•²¡X$¿?Ú·%åÁþ?È¡†/nT¯?ÞÙb¯Ò?¶y­.f?¯Ö~ZK#Ï?—98¼hü?ÝùWSë²?´ú.í'g?ã^ozé£õ?«zäKºÖ?²#†m'&‡?•ê³—¨lñ?Ôº?nÈnt?©ñé'åÿº4FGL J1758.7-1621?ïm²Žªu@aXPÀ9œŒ…´àGÀ;qõ *­S@±€k^@*ˆŸvRm?Å ùIØf3?ÝÁæßóp%@ªò×ùP¹@	Ré¿KÚÊ?ïÓíözE?Éà+yUg¿æ™U ÃÄæ¿è	ÿþR€Ö¿ïÿÿ^ðP`?îÈË ÒÈåAGNbcuAT20G J175841-161703?åÉÇÖ£4?ǁef?·Û.æf›?µJá:oÌ?Ìî%mr%´?Jš†_%?Ï xÈ
A\?͇•º¯àß?ÓÈ	8HkË?Ï:'‰u?Ügºc²sˆ?Ï+£±ƒ?×­2Ø?±#KRûy?ÑÖT5¢?±Ir×P_?×K¦˜é†?¯~ʅ8Y?ֈ÷Z|5È?³¨}Œ¼-?Íã¡/b0?²ÌÏ^6äB?څ8
Òº ?³øŽK+V4FGL J1759.1-4822?Ô±/QkÀ'èE™gD³À9€ƒmÞ*À;úŸ[zz@Õxèt3@µJd¨ E?¸5hÀÞ­?Â5záº÷@©]'«Ž@;;-Ržˆ?ïý› Ø<¿×ÈIe#Æ.¿áñ"ý…ý0¿ä€|â©­ä¿çåöÔÞF¿ïÿö?ŒÝÉAGNbcu3FGL J1759.1-4822PMN J1758-4820?ïì7£‹ÄK?['æ¦ÐCÓ?=émë8z<?7j͇õÖ?`.¶Ô¦?XðØ%qR?ï¸KxZì?!œ|ܲ?5E'Šc#'?X³è¢<y®?BõTñã5?³'
/'?îcõ7œ?'Är$¼Ž?³þZ4D9?uê#Þ
Ð?¥S¬ï±æ!?Ž2ø¸äš?ïº8j±o?h‡\ùC•?P§ÇDoƇ?@Xã¦úÒ?~¹ØÖ,†?g"uìlé4FGL J1759.1-3849?áñg>†+À«Då^³À9¼~Êá:BÀ;Ñ E…EO@³WÞcM,@pöºÜà@?À×&B	?Öæa~?¶@†®â:¸@Æïp:Ћ¿Å«.1Z¿ÜR€ vÿà©
?ƒ£Ž¿à4æÇIÖ
¿ïø]߯' ¿ì#;~†BÐAGNbcu3FGL J1759.2-3848NVSS J175926-384753?Ùö-'{"?ÂA­Üã$.?Ø÷͘à#'?ã™K',?Ê$
H'à?¹ØBëՌ?ÙkTÈd÷k?Ì6—"~ƒ?¿ø1ÿ2'S?À~ØtÂ?ޖž·ÎdA?Ê΀ZªRÙ?ÒE•¼Qà?²‰Böw§"?ം®tü?µ‰óBÈWS?È¢Ìd¤(P?§çZkbXN?㴖ÁÁZ?§‹çZ
†?º.,9ÿÔ*? R‰$d^Þ?ÒGmýVÎ?¦¦`†ÓÁ™4FGL J1800.1+2812¿ê''"-ý@6îð8⟝À:ôSËY/FÀ<›'pˆ(X@ î»J™VS?þðk®Œp?ȸLHß?"ˆfývI?Ñmâ=ž@ÎëØ֛X?ë,yÀ¶>¿ç›¸䆨¿çî°ýŽ`«¿ÚUã ÷€¿…QU)Ÿƒ
¿êG¶þ.n¨AGNbcuNVSS J180002+281050?îáÊ¿³È±?"×͗hU?VÝJ>&\±?Iß$ە€ü?¡,i²ÒB?"'øɎÁ?ïÉå#ÖÌ?›é$ÍFŒ?Vw(ìV?q"Š¿òß»?›ækèý'À?™ø¹,g÷?í®¥¹Uéè?"Í'vÕ¯?qÔ
ó¨?\?&BKgV?±y ˆя?"
pÇ:@K?î#_+ŽeE?'èó5&Ä?]]:\ÓÚ?Tï0´ºÄt?¬ß#r–Å	?"Û&Ì74FGL J1800.1+7037?ëuBµÀI@=·hß½jYÀ:Ê,"ÜÁ7À<‰ep!@ ̀Pó8?ÿCxà¼mÚ?Ë+ëb<á?Ã;9&b?õàoP–@ôe¡o{ä?àœ)@ìt¿ã4>Kë¿â¼RÌU®ˆ¿ÝÜ›Ýk«¿êøU|3WE?´.FåA¸²AGNbllRX J1759.8+7037?î:'þ ?Ÿªëëu¹ô?uRËò"v?nRƒN;×?©³å¶—ºŸ?žEÒZÑ>]?ï;U´Îš?Žg9ø»i?\fÍFˆ?c²%³ïs?–Åì@iX8?ŒDd…YÄ?î
vŒÑ?"¾‡Lì?x¡äC––?j£¶}´?¬DZ¶ž¯û?'¿Ù?îe;6åù?Œ§(úÏyâ?€À#‰—0?n£,@n?©Ù£j+À½?Œ2	,«¤˜4FGL J1800.6+7828¿ï䌳›è@=‡¤¤—À7£>d¿9À;‹Àò£öë@ò@/E@Dȍ$@?'ÃX&T?¢eÀN9H÷@(T<j@™ü)ܝO¿ÎŠ'ûG‰¿áñ<ÞC¿ãΉ/¿
l¿á؞AŸÁ¿åd]½ukè¿év"U:oAGNbll3FGL J1800.5+7827S5 1803+784?ïÁ×Ø¥á?sDªI>«Ò?7Ž…Œ™sD?0Ȋ¦s­»?}›+TEæ<?rép9"N<?ïQÂßMß,?š¼ô?^7ï*—Ò?l‰¸ƒÙ¡Y?"ä%#š¡h?˜š[nœP/?ï)Œ¹ú±ß?Š"IT=Šä?s¯£¾ð?q–Æïö?–<×èԈ?ˆƒ[øj1Ý?ïÝË"Ÿm¨?`7ÂèV¶Ÿ?MÿŽÕqÃÄ?CZ"ߨ'™?j´ù«5æ?\"g'5W4FGL J1801.5+4404¿ÐQ¹1J¶ï@;Þüz9'À8±5
þÆDÀ;ò×DÁ@~$žÅÓ^@uçÈѕ‰?¢m!à?±ž©Š@µ›"/Õ±@§¬áB¿Ñ<&âAþþ¿áÀî<‰K¿æ¡¸í÷­¿ã¡ a}ï¿ê+h{¿åQU]*AGNfsrq3FGL J1801.5+4403S4 1800+44?ïu+&Â1D?"¿_K[pã?[7ô;•?U'H«ò?N7ȼ±?"â.¹µÌ?ïµ¾ñ)?†ã²Ú'þ?@¬×Æz´?S³kgp?±'ÇX
'?…Ý}‹Áã?îËuøDoÏ?'ò†­u?x÷Ǿ«ðp?m~ 'HVî? )§ƒã"ö?0Bõm7?ïýV#¦øÏ?'4™¾?öG7>ùvN3B?2ðØR¥i?%ºAânh4FGL J1801.5+2123¿ïp°ÅÏF@41GàiaÃÀ;½ôµÀ<Q )k3U@7œ9Üñ@ƤD‡?ĵ¤as¸¿§YÝÝÒj?å\=îx?ý3="šÙá¿¿—b¡y¦¤¿çí÷­K'¿å—ß_¡{:¿áÛ`C6¶¿ëOqºû?Ä}XEff'AGNbcu87GB 175915.8+212212?ê*"ËÛÄ?¹¯,Ãè}Ë?'+"	z«Ð?'/^/Œ?Å2_‹¡;s?¹$±¸p£?í'së%ÚL?®røY…¸?†¨ÄL«Ì'?'ã@"þmÄ?±H;´?©C"W:‡?ìÅ»|Þß?›"lSÛ.´?¦ÈÜ
?hû…¶Q£?µîÆ'?íƒ?—©Ê'8ûy?é_—çõjò?¦q¥á¡­?"œ{£Z?~•£2«)P?Ȉ^fbš?¥ùØ(O«Í4FGL J1802.6-3940?ê•R#۞ÄÀ ×d­ÿ',À7†Ã!À;/kn
#Õ@÷ZšUVI@ºÞ¿q?›0œ]¡ÏQ?Àƒä%®æ2@!+ˆ‡"ž@ –žèc¿´õ¶6ˆR¿Þž K¿åH'NI9¿å±Wü@X¿éLõ‰¾¿ì¼Ý5МeAGNfsrq3FGL J1802.6-3940PMN J1802-3940?í¼Ç÷Op7?¡ÜöÙ£Y?!}['k8?|¤;›?¯ë!4?!Ì? šÝÛH¤Ž?î¨ð™Å®Â?²#ëÜì_S?Rk¡ð" Ý?j.kc©Q?¤Ý™T rÈ?²Ü÷‡)?îc[³y(?˜fÉS<§?'j¾£Ë*?Œb÷3û	?¡ZòâØm?ØÜ}	?ïÔÝÓh³?io^ð´X×?=±KÌÓ6P?6ђžÝ?s¶$óW?h¬¨ËšÒŽ4FGL J1803.4-6510¿Þ %šoŽÀ3¤çÝÊKÀ:Hð3Ú"À<')H>@åWáY@;hê?ÀyYÑÇÞ?ÁÝÀåãÊ@Y%5C¯@»ž;¿É¯?Ð$¿½o·ž¿àt•žbV6¿æ~|§ñK1¿é\VbbJοâonLå¿ïÿú@ùDzAGNfsrqPKS 1758-651?ïÜ_afx?f.J^÷¯?O	ܯ'1?G¢	ä"Ð?kÝër´û?c:Nëõßä?ïb wÃ4#?'Š•J–Â_?SłFë>?fÄÏ!Z¿v?'˜æeÅ?›bI4d™?îôgŸ¨ ?…ø‰Ç,†¼?r)œ†ƒ[Ø?bÈ_1MÆL?œè¸ªj%?ƒÔV駺R?îfT1ú?‡	ÇꑀX?|cæEI[?eãȐª7?¦²`%‡G?†vP¿C4FGL J1806.2+6143¿ï–OÀ»$@<ô¡7óŒTÀ:­FBÐ_À<ˆ¢üïªG@Y€Œ­M@ÒÆü©3k?Èg¨Z҉z?ÉqBãTy?õÏíé}¼@ßÿ/ögÑ?âXO'RÑ¿å9ž»'¿êi8"†<Æ¿êpBóš–ð¿î¼üJÈü¿ïÿø¨ó©°AGNbcuTXS 1805+616?ï¼·Î.Î?w€㘌,?iàĬ¡ñù?h'6—ÚBÀ?t³¶'  ´?p¡ aG—«?î¸(Ê؇¢?¡—bÀþ@?t¼°ÿÚKâ?'«¡UDW7?¡åÝ2|<X?âd&‰Ô?î›=0K¯³?Šn8ê¬?xR&ô½ÈX?gþ)ÏLµ¿?£Aè­K³?‡Aj?îÌÁXôC¤?"¾Eð8^@?Œ8'ÿ·ã?ulö؈ˆB?˜K"a﯑?.<‡ê¦4FGL J1806.3+5345?ï~a½4So@<²[1~þÀ:‡Ç™kvÀ<oaÊsc@³IÁ?%@¸;Ÿé?À×Î.äð?²Î¤¾:ã¬?íü¿øÓç@y³Ž¸?!¿æÿ'æFñV¿Øò­œ…Ý$¿æf~ºC¿éQæýz"œ¿ãI‰›á¿åݖ^%ÐAGNbcu3FGL J1806.8+5346TXS 1805+537?ïï7ÑÀ?_\¡Þ¦@ª?2$ôóD|?,^‹)_38?]Õà"®9?]%(T›š?ï»\iK—?
X2a'??G	Œå§×?RÇð¥ýM?€.­`¸íL?|áo¡÷?ï…<ÇÇ?ƒ¦˜¥5‹þ?r}»úô0Á?h<SGIû?™oðÙ©úõ?9cË7–?ï¯ juX?k½÷Õ×!?\>4Ø2c??H=ùwó‹?€°ä\]w?jØÚOŒ©4FGL J1806.8+6949?탑qä!@=*½¨!óÀ8
|à%oÀ; ë)¯%ó@®MÈ_Ö@ñuù`¾?—òu"§¬?ª%û÷:@®›aöK@ÄÃb벖?ïý6Â3엿àùÛ=¨×û¿äõÔ-^'¿ãe.Í/ô¿æ].yÖ¿êo¸õs~AGNbll3FGL J1806.7+69493C 371?ïÙb""T$?p¼¯.gÉ,?C+pJ?AdÔÔ~!ù?pëØHU?pÆ8ìª?îó$k?4™? ^"f?À?oÕ§ç2e?€"Ad‹@ð? ½µ\†¡?yƒ â?ïÀĔ¡?ŒßyÞrƒ&?x»
r-È6?tÖx»$?™y$Ðò9þ?ˆÙôÁžÙê?ï-Ù«@Àh?ƒìû£Ãä?Š/ùü¥•?}rëPn?ŠZ‰5Ó@n?t1ÔíóUÖ4FGL J1806.9-8038?݀IQëÀ8öt)ˆ<À;Vm¾iÀ<±>K•)È@ á'&³ý?üþ¾œˆac?Ñcz"ÛÍ?ÆqLN÷?õ,JŸ`ƒ@ƒ»ùë¾Õ¿éÓÂõ³uä¿ïÿ½ 	c?ïü•¢i!¿Ï虚eG¿ìTտ到?ÐÑ"D¿AGNbcuPKS 1757-807?ï<ª]Ö?"6Þѽ@?ZªøRõÁv?UÀ'¾ël	?–ÓÌå"é"?'(Æ̏Õ?ï%a+¸~?–oB$G6?T|K7v?aBi¦Ã8?šú:<Ð?•9ÅZÃÆI?íŸ1hE]?"Î뛺Š?†²®HGæ?}6™r³¹?°0"ôÌ"?'<÷_ß0¢?í˄Däµ?™ü¼1Úvk?h%чÐËþ?eŸm0…W?°â±9šS÷?™_`ì¾¼04FGL J1807.2+6429?ïMb ±{c@=Gb• ŽÀ:øã`'À<רª˜@ !
]¦ú*@¿»lR9?¿
…&}˜¿ŽöjÍJÃj?юÖ<b0ø@	¼‡°8?¨šák.¿ÛJÿ"	•*¿â»uÝök¿Ó[<'¦¿å0¯?ž%š¿ã}|BםAGNbll3FGL J1807.8+64277C 1807+6428?ïõ#æŽÒ?TÅÖ¿Ì'À?,!"9y¸l?(÷úMŒæú?R5'˳%ë?RÞ*ˆÓXÜ?ïÊæ³>bÈ?~êØìÉW?6¿»¤z?I¬ aáG?y,>dÒáJ?|» ûaÞ?ï.—å)ۏ?€jp;¶‰™?a¤«'±Y?M'"Ü`?—ømøT8?qß',,ž?ïÑH‹ R?_'€Wc?KÞ<ʐž?6úb™€½†?sø¢òք'?^¼p†ñ;õ4FGL J1807.9-6412¿ïðÐm"À3ºnCªy¼À:Mð÷3©À<Ò¡"$@b,™!O@Lë]±‹ÿ?¿bVz]?³,Û§?òö`ÿõE@ÿ@±K ?ïÍ>¬ãù9¿âĬ½bÌ~¿éñ9ÉOiË¿ãRžÓ•=ê¿èó2ýƒMþ¿ïÿôÕ÷AGNfsrqPMN J1807-6413?ïèÜ	Õ¾?]¢ Ì}ÿ?G6?.šà?@‹l€"µ?aVj/™â?Y!ý"Šì~?ï\'§ü&?–³uÁù­?SÖ@ø±M?d•óÓ?"0fðùD}?•ÐF÷ԕÓ?îÏ¡D>i?‹h*2?qw"+ªãã?dùS!M? ×	ÖF¼ä?ˆÖo"ûX?îùbr?
ôX4ì?{Ãú®ßê?dÞò5®?«Çê–Èò%?Ž?æNȆì4FGL J1807.9+4650?Ù·Ž_‡W«@:'ú'è},À;*ƒì‰*·À<Êˀœs@ 궦oÀØ?þW§6:N°?ÃÁˆ5™¿^…'Wîå?–V»ÅàÁÄ@K\YQ?ïrÿ0Í'f¿æþíþ¿Úw
"˜±<¿ÞÒÕºÝ3¿ÞJžß©žJ¿¶ìKÿC'ÙAGNbll3FGL J1808.0+4652RGB J1808+468?ïÏ_6jƒ?oъÝöøB?AûâDéââ?5ÈRÍé,?vè­-"?n˜7rѸ½?ï<ôŽ®?"%aDç³Í?Sאü¤Â*?bþ—7I51?—#õ.¿ð/?'RJ»«?î-"X
tU?ûÚÿ±?r²çvÑj?Y)J~ôc?ªå""iàˆ?ŽeÐZ_?J|­?‡—ÉJ×1Y?m!y7ŸÇÁ?[ºè§?P?£äv×Þ8´?ˆHEû4FGL J1808.1-5013¿äFp6ô³ÇÀ,.ŠqÞi­À:Öé†@÷À;ûŠŸb0@fÀ'¢Ü@‰ÉºÉ•
?¾r]?¡+?¢I=`³žþ?á±+6½+@MΛE–¿èÙÞÃð/¿Ù…=jĚ¿é§1½gT"¿çÉóïT6¿ÙÙÁY|¿ïþµ}$îÍAGNfsrq3FGL J1807.8-5011PMN J1808-5011?ïé,Ӛ¦9?a¬§¯º¸?<˜%ÏJ`?:G±'?»?c@'«w›ç?_Õöž®
ƒ?ï¾>3ïÛ?"áD"
ƒ?2ˆˆ6?Rž¯‡jé?¿6äo'?ƒÃcÓÌQ×?îŠhên2¾?Ë2?zNÙ7£þ?pQ_63f"?¤–7µß´?£¡®¤­o?ïYȖÄtŽ?xF0ì!Ì?Où3gÚ¨Ä?@­îý`·?"Ç#Œ2˜Ø?wÂb[4FGL J1808.2+3500?×Ëãî§h@7uø>ŸÀ:&ÀMb‰bÀ<=JYPÔ@,'úÅÙi@ÿ:Þ"_¦?»7ðÝ"Zs?°_y[X?ó;ëh™@	âæk"?ÄZ÷ÝǛà¿äIÜݼY¿ä&»‹[é5¿áHí¯›d¿ëª¥Gá@?—Ÿ÷y7AGNbllMG2 J180813+3501?ïbGӍ½?£#XÓd%?w«Š¼ØÛ8?†˜•/xF?–¨ÔVX?œ (2Ê$?ôhئ?‡}ˆ÷!Îa?QCŽñVêk?]äÏ_Š…K?‹éžù<?…™Í Àí?îkš»–
ù?'òÏîï?"O´²$¥?€5•"Ý?¤2g—N?×Xtä?îžFOº*?ƒZ‹b*ÛÞ?¡¸^ëž?i]馞wž?¡³0ãIuÚ?'!à™Ó[4FGL J1808.8+2419?êh	Y"–@3¼c¾ì9zÀ:Ïì""9À<XÕï‹=¶@ D›—ËŽ3@ð+[Î\ð?"J_Ÿ¢È?(BŒ;À?œ¼bØxÂ@1øûÔÍ!?ᅥ",˜¿ë…ë1;â.¿ÙÍî \+z¿è/V•8¿Ä FÜÞ<â¿Ý‰/žÔAGNbcu1RXS J180847.3+241923?ï`Ṫ?•QeÚ6w?[d!¯b?T#e£]T~?ž½Ò¨ö?"Öòç¾´z?îк
r"?¢iž3‰Å?`Q£=Y¬ž?plìÑ,ð?¡ï;ûƒ<ö?¡P觞U*?í3Xc¸¸ÿ?™F,øV~?}aCyɂ?lŠxÅir£?´(ª¨Ûp?—£`#³Ÿ?î&I'ðŒ¹?';*揰?`ÿ­ÔvI?WŒâ
-F?¬‹kó¯Ïë?'?ì	z4FGL J1808.8+3522?çªÛWÌg@7s²$ªÚ4À:ß\×qk}À<u¯§"Y@³ò ™R¢@EĚÏ#¿?щĄ©Èf?ÚPÓ!z¤@w|7‰?òI"Ž³°¿Àgّ×-?Ѩ¡ÿïŽï¿àx^졬¿à²öañŒ ¿è»ã?ÕÙ¿ïøbý¦3†AGNbll3FGL J1809.0+35172MASX J18084968+3520426?èP†½Cõ‹?½4^¹4û?À`d¬È$?¸§Ð¸Võ?¼»†Ã`?²5Ҍ
¢?ۂ¸ë_6?ÎîîŸ[??ڂˆ\1
þ?Ѓ Z?Ãõ}pß٘?º{d+¸ãÇ?é<—-RÙ?©u×í´"
?²ê(u7?›GhfïÏ£?Áþ.6·?¢±-©^{?ÑðÅ_ÕÀ?¦tØ»ƒ'ñ?ؔýq…ª?¶Kà'½ÂÓ?Õz=n.¤–?³Šßi¨gÓ4FGL J1809.3+2042¿ï˜ë7µ¾@2Ao!öÊÍÀ:>Ï#¿!éÀ<VÇM1;@†Ò£¦bÖ@§—£öî?º£ÅA"¿w8uKï?¾]‹¡^_@Q
9òÑ?ï\6f¿½{B*8¿àŠUú˜{¿ã®bHŸ¿Ömt¢"?¿âG àö$ŠAGNbll3FGL J1809.4+2040RX J1809.3+2041?îM"zíšÂ?öCìɅ?x·x[ëh¤?qšoޖŸ?¨ÙE¨æÁ?›ÜqæSÅÞ?ï®a©4O?•µ(R}t?X÷wÊ8ö?g&Ð*®þ?›Z¼N8²˜?"ÁCýʂ?ìæh<ËUN?™)-•°`?ŽÆe3%?~aJm¦?´óñsA³?•¤;ž?ícãÐ|?'þBpÃ;?†p¦Ù<"€?s¹Ke\?²Òì±é—?'—'oÝ4FGL J1809.7+2910?æñ·ëòµr@5EV:Ÿ8?À9ƒ-±éòxÀ;í.I¼â@ꊁù"×?ü3=D.-:?µ'‹>s>w?¹Æ]qö•@Xå>³™ö@YmÇXÅ?ïàCß銿å×Ù`.¿ÓcY%¯g¿×#¡šÄçÑ¿áa'·'I¿á€0q·ÓAAGNbll3FGL J1809.7+2909MG2 J180948+2910?ïéô¯>Î#?XG¦Pÿ­?@ЍØÌäö?9¥š'¢7ì?a×-Jþ¢?UÂófÔ¯?ï'rÄÊd?Œ J&VQ†?TZEò€´?eë³î?ˆØ,ȪÜ?Š	3guKI?ïH¹é??ƒ,ÄùÁÈ(?q\ŽP0i?d
óÁ†ÈE?›_Å.Öò?€ð½)6˜Â?íù—ô'‹ò?°†Û"Ë?všäޜӼ?^wÑcS?­"$¦z?U)›G™64FGL J1810.7+5335?ï×l™Âo@;i_JsÀ:[Þây|À<'d}Xs@¸ŸJ;?þ¸\'·ÕÅ?ÂÜýŸ?º>—ãåî?ùž˜5@ "ô>?ëf?úìÆ¿æ‹vÁ¿ã±MëE]Ø¿Ñ¥øã?ì¿ãÃ?»òn¿áAÝ¥¸AGNbll3FGL J1810.7+53352MASS J18103800+5335016?ï½"PGâU?u[§ãôžÒ?ZWèÏý?V0Лf'?zØݨ??sª+g`ä?ï*†'?"¼ªLA.©?i-ê,õo?sSì»>?š–ÝlQ?'-󏽍í?îÎíä»þ?ú?ÁXD?{AóA–?ñ?eµ;ýŲX?¬ZÒ¹x?ŽÝ4të=?íá[ù²?Ž¦ÐœT¡Å?—ç	þÚ?~ñ¹È6€!?«eάe?Šóî`ÊäP4FGL J1811.0+1608?åËóW"Ö*@0ٜ¾èÀ:UáE)Õ¼À<7tm&S@ •R&é?ÿaýKÙÆ?ÄTPåÔÝ?À¾õHÁå¾?üŠ=Ü¡@
ÐÏ֗{Ý?é?÷!	:¿ékÞuk¼ç¿Ý¡ ñ§£¿ÐúBœÜ=¿çÎ8§ç:6¿å´ ÓʘAGNbll3FGL J1810.8+160987GB 180835.5+160714?ïšâÞïå?¨]2‹Í	Ä?KÉ?°œöÿ?FÑU3?‡Š´Hüïç?¨_HFòV?ï \w­?†'P—ìNÍ?Bsþz«%ð?U‰ATZ7?†Á¢4jØ?…X‡`,œ?îF	²ªG?"6¯Ór?qqćS?aOû³ÏŠ?©qD>dq/?"WÞEX2?î²=iwi?"B |>'?kj^#m÷ö?V­Sá²=»?£%ƒ†WÚ?ƒù~ZeÝ4FGL J1811.2-2759¿ìT˜ÝÿF"À£D^Ô¡­À9ðb¿¤À;¦Ù>Ëê@ r%|ç1R@
òœj.r?ÁÅ[¿Cw?£P»¯C$?æòûE•‹@–šÆÀCR?ïI¤^ïz¿å¸ýÿÚ¿åìŸÀÐU¿Òõ¦n"2¿ä›…AÚ¿Û``="(AGNbcuNVSS J181120-275946?â§ÒÖv1?Áé€Øw€?t:Úsö½æ?gê}mK¯?Ú_néCÂá?ÁåsÄ ™F?Ù­êïé`?Á¶Z¾&w¹?fC¥\çN?s²U"ýhA?ãÇV+$?Á¶ôbŽ"?ãí£""J?²˜šbáL?œ>KœSª?'"Ħ±?Ö`Ô7žÉ?±xsMëÖS?ãå<…?«àöà3?'‡'¾¾3?z'¸?׬Çáá?ªûᛣƒ"4FGL J1811.3+0340?ï3ªXrv¯@%4¢v·íBÀ9-Ôx'¸ÕÀ;®n@O{h@ßqÎ#Žû?û±ëºÎ‡?±zƒ(éÙ"?¹£Íúõ)7@2‰¥/ÏÑ@ ý+¿ïÿýFKê?ïÿàU?Íu¿Ô¼Q?Û0¿×a!§¼r¿ß
®ñð¿Ýî–áƒh*AGNbll3FGL J1811.2+0340NVSS J181118+034113?ïõÊ.üf#?M‡†@¹0?$KXc¸?·?oÃT?Qâ6÷­??L
$ã1ñ4?ïS|ϒ•G?žŒ-ª?TLK:Ÿ€?d+p3ð?"PHù­$?­fúí²
?î+Ü;ÆáŒ?"Έ¤Æ?/©–?{/	qÎ_Ë?©\G#eP?'=¬9X?vð8†?‰³Ç<äóº?u…è£5'?bØ:Qî¹?¥$è?ˆ¿:‡p4FGL J1812.9+4249?àyàN3ê"@8ÅAt>–>À:–´ -œñÀ<g&••þÚ@¶-÷ `@s¤<ŠÊÊ?Âù©d<ën?£ªËñº?ß)í9SÞ¤@q‰¢¬=?ŒUe­È"¿çÏ d#–¿ç(9À.e¿çê	*v¿äµ`iÍ#4¿ïÿäâBTäAGNbcuNVSS J181308+424853?ïOòtv'?‹ÜG5"'?p¹SBNê2?h"ýc>VÊ?'Ó\ ©U?‰*ó+L?ïnÝ,‰¥J?ŠüFrb·&?Qšñ%'Õ¯?\z…¨§ïë?'
«\r)_?‰óÏ>ž(?íîâ"?'rOÖK¡5?'i[­p?qIBs!1?¬"ðö'¡à?*"·1Y3?ï!f)¦•?y¦^Hž‡?tバӫ«?_»ꬱ?–šYæørà?x5À¹;®4FGL J1813.5+3144¿àø¶á7Ò@5`RÚšÀ93®üm¾À;Êù²Þäý@çƒzú@E"FK=ì?¯‰ðÚB[?¢èׁÜ9?ôÌF嗞î@
KH¨»J™?ïñè°X"¿åT}e†l–¿Ýs>#§$¿äloàŋ¿à—¦°'«¿åbf'P¢AGNbll3FGL J1813.6+3143B2 1811+31?ï®Á~XÏW?zy‹˜þÝ?IùX»^?B'Gü\Jà?'½°ÔKÎ|?y˜X&×·W?ïŽacÐFz?ˆax8‡pó?Qî_êíYŽ?aªEUï¯?Š)ې¶"?†¹²¨ŸQ?î¤U©Šþ?«\@?wîbpM¥?r<$šÑ?¢¼áû;?Œl#áôe?íµ­†
pÝ?"A:¾L‰Ì?ƒ)§¤[?l/=kԟê?¯ß]5?Ûg?'p'‡™ ˜4FGL J1813.6+0614¿î[bIKM†@&xžÛø¹»À9…È•/§À;Û$
¡C²@kىô‹?ýñ ¦ÔÀ?¶•ÄÞýã?ÅyÞonM@¡ÃA2Ð7@	H€ô1?¾¿·ë˜iî±#?ƘŠ:N¿Ô>ðÁ¿ݏO(\?œ¿ä}Ëùï¿çK`6÷cAGNbll3FGL J1813.6+0614TXS 1811+062?ïFê²Äp»?Š[~Tý¾î?ƒÇÛb`ß?^3Dö¸š?Š}Ãsp+?ŠNU²€<?íªð¤ôµ°?³±î´Hü?ƒœˆ&åV?‰!P&©?°4éӖ•Ò?²Ê"/~i?íêJ­u?šÔ¼GÑê?"D—æýÙ ?R"À5?ç?§4ßa©Â´?'{¶ˆvFë?陯?ˆ{? lúquÝ?=ÏÄü?~ËWŠ5N9?Åñ‰ '? ?ŠLCø4FGL J1814.0+3828¿î•;àÆ@7dÝDUÀ;l$ˆþÀ<¤$u*Nˆ@Ùܪ»U@!€[2•?Ãé•Zo¸?€ËŠ#ý,³?ÁQ׎â@…DM÷?ï˗C¿äª¶ÂŸLa¿èo,s%'Š¿×j,#tyO¿Þž^då1ó¿ë/…>BÛÈAGNbll2MASS J18140339+3828107?ï[9:Pf?"³À.x27?TXGÎùâ?H«TÓXµ¸?&&¨r_?"š¸™
?ï‹õ•¨á¢?†ÅÁ
Ö?B?£ZRð?TÚ¢9Öú¥?‹Þ `"hl?…¹s5yz?î`á_/v&?ŒÙÉË]žA?r1`ž…æ?[ÿöÐÓñ¢?§«½ù7à×?‹',­ie?ïO2Ù­!?wo¡
eâ)?`h_|ß"?NŽe¨•Ò?"¢.zì?všš™ÅöÃ4FGL J1814.2+4114?ê£C{w<@8 9GIj­À;²_c<æÀ<…"f+®@ßÁ_±@@h–<"?ÍøU¼ ì?¿ó¬-AØ?ð+uϏö@Wâko°?îQ6ßD—¿ÝÔäžO¶Í¿è08­¿è´" [Tº¿ä2ÙaÒ£¿ïÿð`OËðAGNfsrqB3 1812+412?ïŒûZÄb?€‰ü›ëq?`Iß°x'³?W3¬Ïx'ý?ˆé‰=0Ã?f%½çRv?ï,ó'9Í8?"+™ÇGžG?a-ïbA)¦?t Ûâõ\'?˜;Ý,~3ª?'Á̕ÖÁì?î/Ï´àuM?oGþÄ?{ü8ív¶?m'L+Œã¹?©ƒ}"IÔ{?Ü¿xÐÂ?îӰڌ%R?ƒ™ÁögœR?t~ÛÄ}Ž?bŠo zO?? 5÷.?'øXEJò_4FGL J1814.4+2953?î?—Ï·ZA@4¹à`þHÀ:œÁr%·À<1ýKÙÆ@¹‹cÅ@EI@»²?Ņa(c÷K?³ÄÓÚGó?ìö®G¦‡¿@
è§á6¼¿èIžŽ‹t¿á< B¿çÄä þé¿æô,Ý®œ`¿äª$+X¿ïÿ6a;aAGNfsrqB2 1811+29?ïïۆÂô?RÊ/–"—E?4ŸÔ%k±?+…'F}á?[ þß)"?Qq%^w?ï­O''x?ô6$ŸwR?E÷¢På¿«?\ª¤aŒöL?ƒL¼Í?€wƒÇ¸|-?îÖSG°¯?‰¦UÜ22Þ?sís$Š£?j$:s­é?  }3£?†ZéxPx?ïjWŠæè?wbY@ù¶ä?Y	H« f(?IîQ¿#?'$zƒÜx?vя#´£4FGL J1815.2-2715¿‡¤šXÐ3†À_óÂîÀ9f}å,õÀ;7sx @=ϕÿÜ@®ï¼»Ý'?Ã_À‡'?Äÿ{á!îg@±ÕÝ톁@~žHªé£?ـR`J¦?íØRÂD³Ž¿åþ‹÷§q¿âÊ¡yaë­¿ç&r@T"¿ìÔ(᠙hAGNbcuNVSS J181510-271304?Ï	ACJv?·óº·)#P?ǜ¤Mwž?»öyfDó?âV†«h{?Âao{H?ÁkªQ²o@?¸¸~°G?Àæ÷%ù"?ÁÏýiw?ç Û­Éåè?Âý
`Gå`?Ñ
¸Šåw?«î©%¡kÑ?µöK¯C?•>"‹!÷?äºc'Ä­?«ß—¹É‡™?ƳÒ叡? ÍºÃ b?ψ®Û•¬?®
ÒÓñ^?âpߏÓT-?­`S§4FGL J1816.9-4942?ÙZã°ÿ£À.U¾'bEÀ9¡ÑÒÆÀ;ðH±I¹‡@mÇ՗ Ã@ôÉBԐæ?¶Í¬½?Æ®÷ϯÖ@Ðì1"@\ÁÂ,µÁ?ïøè^£¤_¿ã´¼j~ùÛ¿âqÚ}ºjõ¿çƒüÿšs¿éâ@!-L>¿äÔê"H)dAGNfsrq3FGL J1816.9-4944PMN J1816-4943?ïŽê@ß5V?—1z±@ºù?rÚþ']?Ý?|n€sɇ‹?'×ð"
•?¿sòÄË/?ï½Ð2?‡üÁ­²?9¶§XË?L­Ÿ¼Ý]2?ì¬|‰rC?‡œ}ÎkN3?î]ƒÖ-?"'§H€šB?ŒŒRžñ¸0?ƒip"?£ãáß?‹Z4ë?ï'ì.ý?zl
h+ºV?júQªXw£?VŒø*.5?—ÀI¯»?xkÈS!4FGL J1818.6+0903?înt´ È;@&¸÷QÕÀ9S€éŸkkÀ;¨J¶Ýw@÷—´&¹@#z›§Ó?µ8ð6‰T?ò	½n
@
Jè[žŒ@(2Oˆ~i?ÔÒ«3=¿ÜºÂÇ;=¿å?çÁŲ§¿å{C؜䨿èeçPÑÑ¿ïÿ5Õ¤â£AGNfsrq3FGL J1818.6+0903MG1 J181841+0903?ïÉÃöµäd?v©v°ê¹?X½·
\ɬ?Uۚþ"?tî–ᶛ.?t'–¡ž-?ï—{¬–4ž?³o8÷R?G´rpG?\á4zs?ˆ°‰"R±|?Žñž€¡É8?îQV
"&?'¶1Tž*	?ˆšàûYĒ?|ë>$wb†?¤ÃÝðP\{?ŽTîÏš?ïIVc֍Z?|ÅÄõ?c"¨¹·ÎÙ?LÁy§Õä?"pÞm÷[?{HÄD²[ô4FGL J1819.1+2133?ÚM\ù™ù*@0~ýX…ÓÀ:P-zŒŽÀ<L|tÅ¥@í	Yp	@tw·?ÀɤyF'á?ŒkÕÄ ¶ø?ϵwß?øüyzë-¶?òÉâ¿è,YÅn3º¿çe`¬é¿ÊU?øh†ý¿Úð®=ës¿ê¨U¿O5ÈAGNbll3FGL J1819.1+2134MG2 J181902+2132?îŸ?Xçš?š›ÑÍÚ?nÇ*0µ)À?ccãÁúˆ.?¤—к3Æ?™Ÿ–A`?í?JÇu8õ?¶ÎוCµ?ug`'Ò'?~% 	}9ï?´¯3º}-?¶{÷'·nÜ?í#f‡«GF?˜|ÿ#fÃY?…	£iA‰.?sŨº*Ù?´C—U}"µ?–1ñÚc•Î?ëAú§~†Ú?ò÷•?›˜Gݺ?…&>Ó~Ñ?¿)D½ùѺ?›˜óoÍ,`4FGL J1820.3+3624?ÞÖRè/SÖ@5Þzt:À:"Y~À<ƒÎod;ê@ èíˇ'?ü5ˆ]13?ÂêÄ.˜š?§%E<}½N?轶ÿÛíÒ@½rã¢QN?ïêÒa6PÊ¿éV!IÑ°¿áãп "`¿Ê"~èx~¿ÑÐrß­*¿ßlg1gAGNbll3FGL J1820.3+3625NVSS J182021+362343?îêEüƒ?–×rÅÙ7'?`Q·]–"?ZzO'Ú¥ê? ^9@*^€?–µƒÍ?ïz퉐yY?;S¦Å¹©?HÒ²åø?TúàÔ?Ä`pÀV?Œ&$TÏó?퇑†L?–ÓµubR?u8òÂï(?e_4?²oä¡pþ?–J´Êdٝ?îZ¡eJ?ˆ.[­e?oÚªôŠ?\C?Z$?¨d<¦åÚ?‡Ùµ[Ï-4FGL J1821.6+6819¿Ýâ]xAÄ@;Ìú¬Ùè>À9<f0¶1À<"øR@{ó&þœ~@—AЄè?«'ÈûîÃ?ªâðz¦å?÷ÀW xF@9Ê&)?ª
‹ýáB¿çö!ãÕ}¿çÛÓ/½\í¿ècúÿæ¿ëÑT†jí¿ïó'^±ŽAGNbcu7C 1822+6816?ïæë-ôeƒ?b÷㵞ö°?EëÜræP?F¼B¼L¬?c™Úîàúö?`,ÖÞ¯zÏ?ï©/¥—â?†ºö"PP?GπÆ0é?Wü|YR¿?"7A
6øÝ?…l_åÓ?ï"%"Iê?ƒˆàw‰ãU?s±aø?dã:ÀÕ?˜æ®÷/Áû?¹Š¢ Ic?ïÙÅÕít?^C vc¹?Zý#"ï>?K<Õ¦}?h»™3½i?W°ûÄ]˜4FGL J1822.0+1600?ïz't}'@+0Ãóà7
À9úmû†¼À;ä$>úè@‹hÓ©@2¼›&b?ßàŽ¾?ÁjýyèÏ7?ø¥=§*{Õ@(",J
æ¿É]q¾‰¿æ@³^'°Â¿åJ*Æ}'s¿ìÿGþò8í¿ÑfKÄ#°ß¿ïï©:÷LÓAGNbcuOU 134?ìí+P:-?²4–ù½ß?†ÀÀË6aœ?‰Ö¼:#ì?µ¿vŒbd?±~ؓ?îÄúãBZ?¯ý,ˆˆ-?t5-@õ¹?'kÂ~¸F?«½
©­#F?®j*)°Ûç?é‡ôšT{°?ª>G"­?¤îú¶›?'Ñ%%¶Ô?Äßkšïc›?¦ÈÍð@v?í²<x	û&?–ιÇ6|?zù:""×?m*á³xÛq?°¾ˆ—fée?–1èÇôw4FGL J1823.3-3720¿Â««KëmÀ%íîÇÉXÀ:Î/OxäÀ<‹Fí$[)@@nå»Ü@Ô@C¼î2?Ôæ|+õ|?ïÿø]Ê5™@Ç%Þ¶Ú@›ëƒq9(?ïà7]d_%?èïÕ¿èÀc'†W¿ïþ.~Ãq?ïYِ)®O¿ï¦€g™lMAGNbcuPMN J1823-3724?áÄÆlõI?Êø¿ëV?Çîš%ê@?Ãoð¸a?ÑÓo& O?Ŏ"r&Y?â¹DHÁ?Ñy<šÓg?»PEÁ?Ãd©¯x)?Ó©£»¤*L?ÍeþÈ:V?ÛD^ÁÁþÿ?³Ž'çt?Ö*¼…ì?´'®wÄ?Í!Êcp)û?ª¼ÍåT?éì,äV ?Áx0ž"]?³Œj؝ë?¼<¿ãôl?½À?cè?µXòñ#‡4FGL J1823.5+6858?Ð	`'x#c@;«h¾/{À:(ðzPþöÀ<oE§©ý•@vb)?êQ?ÿ…C5ßµÞ?¹Ãy'çI?Ðît1Žî@«>o§X?ûê"Ò/¿ï@)æÙ?ݤQ¦ùT¿àþ3ÂOEc¿Þæþ¼³úï¿ëüYýÍJÌ¿ïÿùµc#¼AGNbll3FGL J1823.4+68577C 1823+6856?̇†•×š·?½CóQ"̓?çq	™tSž?¿¯lÌKÔP?¦ÑL\[:?ôuÓa®?ÐŸYŒEš?ÇîÏãÖéÚ?äÉBqâ?ËÊ܃M'Ô?¿—8†F?´Ã—²ð&+?ËÏxêD2ß?°De΃š?ä‡֖k?²ÒŒd)`b?ƒ»b §?¡vÖè™de?ؤp§;G?®ß"I‹÷¥?܍´&?²nÍ»*äæ?ŝI{Q®?¢ÛbYՋ4FGL J1823.6-3453?ëwé܅°À#ß6ï€UüÀ8¦}¢ÃÀ;~ð=ë@ça•q@à?û(œ6,ø?§}–¦B¹?«ß¤jØæá@+Còž@û´^kñ?ç$çá¦?ïù—02ͳ¿Ö[œ¾'!€¿ÒŽ"&±¿à_ZοԪÂ@ÆAGNbcu3FGL J1823.6-3453NVSS J182338-345412?ïf³±©m?ˆê©ÖàhA?QÉä
š?QV·Vð"+?'øê~1'?ˆ]Öü.ý®?îÕ¡µŒ»€?§íB($mI?]0…˸à?|ÔÔT¯v—?¡¼`xր÷?§=߂s&T?ìâ#‹¢ª'?¢#'º¹½Q?†ˆKâ?~NF=?¶-r™ˆ/:? q‹eGÃ?î9j¸™]•?"Zوk»?Î¾ï¢	?rÊYb¿º?§õ¤º¤r?'W Þëì~4FGL J1824.1+5651¿ã<ߘ<³v@:Ù#d»À8w–Б}kÀ;ÛLg"t@½vá³¹«@o	R
?žöÐ"äþ¿?°'²o~h@§Ó[\G)@k#Bû'S?Ë%=|7^¿ãT"Ö¿å¿ž ß¿åÚÛo›ï¿ç!ueݪk¿å#slß&lAGNbll3FGL J1824.2+56494C +56.27?ïžê‡Q©?Œž¸;²?Wå/×r|?gjTá"<P?…c!…šË?‡­q,ӆ?ï'éVIy?ŠÅÐ¥	?RJuN—˜?]˜$»?Œü[ÃÎÝh?ˆüuÉgÑ?ï~(Ku?‡ê {SՎ?uҕÜsô?jõÐgô¿÷?™›•to?"¥aJöÞp?ïÒhäà–?añÕúTqõ?Xƒ¢àÍ{"?I¶$üÍ»é?pª¤×ÄUç?]R@úÏ=4FGL J1824.5+0107?ëìâ8fE@ÃX¯Ä~À8äB(™|=À;	‰H¾I@.<<œ=Ž@.—eóS?¸Ôž}Y&?²+
Ò&?ô~žš@*êëñ«)?ê¯+ie¿åù	p¿ëgV@S'3¿âT	×ð~¿ë^*Ã") ¿ß&a"˜ÏAGNbcuPMN J1824+0104?ìÆƁ"+­?³™$_ô?yh´íÛy?sCàS=ðµ?¸9hÄè?³4€ˆ¬XX?ëÅÞ¼ÿ×R?¿aWñ­_?pÇ%'Œ~?';4qÀ™^?ÀbLâÔP?¾™6´‹'t?衳"‰û?°€
 7¸? Ýlþ"L?"OÜlz?ÉAÖr:À¿?­Õ4ð²]?ë{K¡?¡¥ôÃŒ)?'ÃiÄMó?zªqÍ2?ÁYI¥˜ñ¿?¡OÞ´ÙÅ4FGL J1824.5+4311¿Üý³0æÊ@6ׅ@FA-À:Ô{bvíÀ<+¼FlÌ@!4Ö½;ŠE?ûÇ(-E³h?ÇWOGß=?´àú@ÎQ\?ð܆Ô@Í:Ó»~q¿è¿!Í°"¿¢I÷<Ynÿ¿æò•^KË¿ß!š•m¿É¦hßè]w¿ã•õôVÿAGNbcu3FGL J1824.4+4310RX J1824.2+4309?îÐ`Œq?"Žga.Qâ?Z2ìUæý?M¦žfžV	?¢.P_Ö?'?"F^pX?îðE–ÚüG?¢p'»0?^‹i›¹=?hl<…ŒÙö? KIó]Ç?¡þ»g×õ?íˈAU'¦?'é媹FÀ?v/Ûg5?l?dìÂ1+}Š?°@À>ãnÒ?'¶wW•yä?ì¥ó'cÛ,?ZI
?{‡Û­Bb'?rÏSdFáh?¹åº
w?žQnלÀ4FGL J1824.7-3243?ç<"—Ì1iÀ"V,UÉ`1À:­_ö	ÜùÀ<"Ó~—¶@?8Aºàf@O8œÿ¨?ь®¤˜¦*?Ùk¯#c²@	ŒªZ±ý>@Ùúf=!?ïʇ½ùö&?âtÒò¿â.ÂöŠ5y¿âcò¸ï 6¿ïôcê‹#µ?ïj¾º»RAGNagnPKS 1821-327?Ó\¦ 6·û?Â|x»Â?Ս—nâü?ÅÔ~EÐÃ?×Âq³e	?ÄQÐr³ˆ)?Ôù"{š?Ë 4LÙî?—yú½x?Ãky²Ú9>?àÝWEä2?ÍYé\±0‡?à,M½C?±þJ½'?Çf!Z†e§?©æó\a?ÓôS؆ħ?©ØêKLói?ß/)xÌÆ?´u)
0ž?Íx\äÏi?´"üXì–"?Ò¨‰wK…?³\õø †4FGL J1825.1-5231¿ïn¨ö¦1À1u;÷'À9N\(õÃÀ;ä(ôëÐ@_êVËhÊ@;šû™hò?°Ù·µä?ÀªqK´´@Òµþ,Á@'dkåV?qÏJ*›Š¿ÙÀ.XØß*¿æ¸÷˜Rq½¿ãõՅØò¿êC7¢®–+¿ïÿ ºöAGNbcu3FGL J1825.2-5230PKS 1821-525?ïÈ[Ú^â?n¹ë•–D?`·G9?W†óXGju?sÌ7YÉGK?h—F,$©¤?ïÚx«Y
?v+N2~ÐY?*IÄzb?>êB?KÄ?qñ\3i*½?uƂEl7?îˆæQY?'Š'i°¤ ?‡'ÔW×¢D?€/<,¬Q?¡´lˆ•ò?Œ'h:ZÃ?ïÉÂÒT"?cìÄ>y]?AÜþWû?4nÔ¦Qa?xãRV-²?c
§¡ÌC°4FGL J1826.0-5037?ÁÑüfsÒÀ0Ý\…<ƒÀ:åCä/À<LERðh@ %ZÕHœ?ý͘T<?ËÏ?tN†?Çó(ªB?ýÒK&nÿ'@ݺÄâr¦¿ïþM"r›©?ïÿöÅĚϿ¬&SUȬ¿ÞøC¾EËf¿ç]þÈs¢¿Ñ‡wã¼RAGNbcuSUMSS J182551-503914?ï¢!àx?|¤
¨?Wv¬>kR|?O=£Ï©ÚU?"ˆê@0w"?{«°ß2hä?ï>åò†æ?"`Þ^R?[Ë®'	Ä?géW¡ƒ?–f†Óî‡?'* |$ÃÇ?î}Eˆ?pF
ë?A?{Iƒþcç5?pÑë1¢ÎG?«eç°* ?‡ÏŠôh!?íÂɵ‰ëÔ?ŠËZ`<1?†Xé¯!å¶?r]êÁ´?®=*;˜ÉW?ˆæ2¬Š·{4FGL J1827.5+2015?|›êΝa@,X–Ý&·$À:ãAÒ2g[À<K§°³''@ N+9>ºü@	T!ÀD(?Ãߥ+Ï¿¥ú—$82e?ã|‰ˆª^
?û9ÐUîI?ïü!ƒÞFr¿å(Gýo¬á¿ãœa?`9¿ÚÑR+Sk¿Ñxâií¿íC·'sAGNbcuNVSS J182730+201309?éÁ	"ñ›"?À0b\4ø?~+Åcžˆ…?¬.| |ʕ?È
{…©?¾=Ÿuúìk?é.³°bw?Èä
¥ë¼Ž?zæì<Èr?Ž*Á­F‡?Ê-ƒRz© ?Èb#Dj'?ìèñœ?£ö^Ûa/?"]`$ =n?r0î~MäŒ?½4³ã»r?¢Îù:•î?èÍ8u½›?¥­zq[u?‹qÕ6ï??‡›ß§Qè?Ëè՚£?¤Ã–)>4FGL J1827.6-4029¿ÛY§ï¦I3À*Q´þzÀ:Ås½fþ<À<Nx"PŒà@Q†QŒ@njCoÁY?ÐP¼›|GÏ?ÝaÅÂÂ\Ü@
•"äþòº@Xâš>…?ïùu'
5ô¿çumjf¦'¿Önà2…8¿îoÝÞm¿éÏÅÀi<¿ïÿ®¡hšôAGNbcu1RXS J182724.8-402904?ë,Y"º6R?¾±âá{çî?¢M4zž?¤Sä1»?½Œ¿ðþW?¹rš½'öß?煀7M†h?ɝ0§?±­Ìú¥´
?µ—F¾Äi'?É¥wY?Æ)H']?åjþ•ìc?­¸|Ã2 ?Á5íLzÅ?¤•ög3(?Ê°f¹¡Ó®?¦[äÍi#9?àú+€zº?ªa›$Vhž?·ež"½f¾?¢N[†ðà?Ø2Av°Þ?«.m>^;÷4FGL J1828.0+2634¿É덣
®@0ŽØ
±À;­î»4À<Žä†&ö@ ¬!®{}û?þ»ë¹!^?Ð ‰ãC0×?É87)Þ?ønã]2
>@¡€\[˃¿ïþR¡ªˆ?ïãë¸J_¿À®ŒDòMe¿áp ßs˜~¿Õj\|ؙ¿ë§A"4ØAGNbcuNVSS J182756+263313?îÄËY0æ?š=þ=ûû?qé-`£x'?j/áwk<b?¡v$ÀÝ/?™2Mýï%?îÙòóÔkd?ÁJmrÕ?g:ŒŽ»h?vñ.ÖX7? í'ùØ
ö?œ:6$¬Q"?íveÛSÂ?–+ºË×&‹?‡‰O݃Š?}òò³h ?±[§)±}Ì?"V»PJú?ìàvp'–?–Ø2‹i±?…$‹ãš6?vªÁ7@'%?¶X‡ên܉?–¤"d÷Q4FGL J1828.7+3230¿ã&wÊ@2Ÿl‹C•À: jüÎÀ<§Iˆà
ò@Í+4Ja?þyŒcP1q?ʜuìì'?äk•ð]Ì@–fœí@`Fë¡Ï?îé}'Ô?¯ ®ˏ¿Ö;™Ƚɿä…Lò!¿ïÿþó…õ?ïGÉÃ-ÚAGNbcu3FGL J1829.2+3229B2 1826+32D?ˁ"¿kòé?Ã1é|'õ?è$\ÁÌ¢ÿ?Äjâ`:Ã{?ŸhAËÅ?¢H²'ÚA?ÐÕƅ<­?ÉXrãv?ã°dF‡•?̼+wj«¸?¿%ú›¬¬?²¸­§6	©?Ïo"Póê÷?®lͷΌÌ?侔8ÉŸ?°pi×Íó+?»-—Ï=!?œMÃUµüÚ?á}ÏLn?á?µ¥cjÛùÕ?Ò%3øȒ?µ7Ö=†v?ÆxfUoX?¨{/ì!@4FGL J1829.0-2417¿é©Æx'¦Àäœ@=òÀ9M	1´®À;™Þ˜§+S@˜#wÔM@´¶býü?³ÒŸt¤í‹?"³n#kŒb?á Ϟ8dË@¼‰¿±Ü1¿åŸ'•¿†¿Ú##´e"¿ãhÆ]Gô¿à6U\Rç.¿êŒÕ€Ðtø¿š ½R¡ÛAGNbll3FGL J1828.9-24171RXS J182853.8-241746?â?ì9"?ÃK
¡?ˆ.'<õ[?~óÈ^Xnš?Ú¾³¸K¥/?Ã"Gä×ÃÕ?ä¹	‰]Þa?ÈŽ'þë¨?c%B+Pý?v7¾9«?Ög¢hí¡D?Çù(…8?åw¹‹»æ?³Îë>6??¥LüÜ
¤ƒ?'·]•ø?ÒfíMßg?²‰l@¬Ÿ?ê:8&?¦µ-"í
?"²ŠoH?}TŽŒÓ?Ķib¢?¥ÑÐ=q4FGL J1829.1+2729?æ}®K"­@0²{åS¬OÀ9ÄP¡C§À<L¥ËD@Ð<Q¿æ4@"îV,\?¼MfÿØ+¿?Äj´iS«¤@¦Ôš÷g«@ã·Shݺ?–tP›	Aƒ¿æ|š…R¿äñržƒ
f¿é¢>Çç¿ïÿ#–Ýýw¿ïúÚâ9EœAGNbcu3FGL J1829.2+273187GB 182712.0+272717?îÌƉ^?¯0õQ8h³?"âJ×¢ð?'‰fîro?'¬2oŒÄG?®OÉ&"‰?ì]ÀëD?¶B‰žáœ/?£HNÊ>›?§W"Ö³?µ‹V"†˜?°HŒ6š0?ìŸ<žù·?¡ÇéárÖ?ŸxžýÚÉ?"°õ?íC?³'óH»ÁÑ?—dل'š¯?êzÆB$ې?¢5Ê# }?´†îO•?›	øóð?·£¼Šã?—î2}»~4FGL J1829.2-5813¿èå	trîŠÀ4j½ãû½À8†‰À;–lÅ%8Ÿ@­ŽE'§d@rÑ®³Ý?œ€4»Í?ÀXƒ#á\@`^åh¥@
t÷"ᬿÑAwcä«ç¿ãÆ°žBö ¿èS]õÿv¿æë+Ý~uÒ¿ìIìqþ¿ïÿî' ÇAGNfsrqPKS 1824-582?ï²_7 †?zwÚÑÁ•†?w–¤ÀÒA¹?vf˜SÙ`?ns¢Fº÷[?egLÐí?ï¢m_	?^Þnö1Ù?FLt«O°k?d¢
ú€«'?|) 3æ…ã?€fNž+@?Ãý)?"ámS5y?•ÁG#ê…?ƒå¯›/#?•Êc•Õ³?ˆ5Â^³'&?ïáÊ÷Ñt?bGw'ß?C'¥7¢ÍL?AÅoD±•?iT^à£5Ú?`åmz™SÕ4FGL J1829.3+5402?؏üöôØ@8Ìñ`®—À9úVÔ"+¤À<d?³t63@ 5q4ˎ´?û©Ø@žUÁ?·*KØñsJ?½Á"o:öK@õM¾Ñb@9{E¼D¿ïå!4y?ï'~ nö¿×—ñ"íjÒ¿Ö9ñ'õèO¿Þ‹}ÂM—ã¿â'«@‹AGNbll3FGL J1829.4+5402RX J1829.3+5403?ïîô@7?S'³ þ²?@ÆÀ˜?<·?6ôåÊWY>?Y´yqfC?PXΪr·?ïŠÓügP?‰â#Íy1?X,¥!Ä5Ä?en=¼
°?ŠElAóQ‰?†W2‹H?ï*èJhN˜?}ð6wzB?h¦Ë	ÎÂ?a †TßÕ?—ŽQ¼jn?z굊¬Ó€?îôÚfÿ¸P?~Zi2:EÉ?Î–ñ˨à?kvø®ÇÔ?˜}g§#!x?x'E‡I"Æ4FGL J1829.9+3934?ÍI"5"F@4ȕá~4¹À:Ðw/†FÀ<šã'áït@HK×Cô!@"ýØ?ĺ{B?·ÉÓH<ç?ôÿ5ºÌð@ê;ò•í?ð¿ä:'
‹þ¿å—Î=e;C¿Ù¦DÉ]­¿ë&i@‹`q¿ïånN'4KAGNbcuNVSS J183003+393638?îÖíë÷~?IÃ=a?q3p1f1¿?lù¾ŒîÏ? j¹ÛÁØ?›K	ü?î=Ur'ô?¢ÓŒeçyŠ?€~ å2?ƒ¸{ñ69?ªLª@ӗ?¡ œK?íH'€ú÷€?˜Kè™Û‹?ŠWSÐùÐ?~T˜˜ËÂ?²hA
®$Ç?"óiÕ»'‹?ë¶Aí´šÁ?—_œϕ,?§8±G…è­?‹[uü¾­?¶±—î˜5¥?""#4ÃíÒ4FGL J1830.0-5225¿ïS"ӝ\®À2ÁLf
À:É20Ô´"À<lý@´%@5ՈJø?ùÞ Ô÷=º?Ö%>}êª?â¯'9*Ä@Ü;\Í`q@@DˆE?íº¬Ùè>B¿ïÏÖÍ׏?î´ýØÞS¿×'Ï<h¼¿ìCÌÞj"¿ïüDôü–¿AGNbllSUMSS J183004-522618?î±N¿ét¤?£Xì)6$?ƒ'"X(=?"·®¹¼Ü? !/+^¦h? ‰«zÎ?î9q«s"?­0«l¹Ù?.…ôL¡?šQî~•·?¨C˳ÉÒ?¥Í`!Ó­U?ë(ÖßMm?¤ÐW˦õ?¡…Q ý1?ŽÜ|ÂXÜo?¿Ãu?¢ea×`?êÃoAsO?¬ÝùMSp?‡\¿>5}é?…è/ù_?Ã|wPRå?­ oÀiÀ4FGL J1830.0+1324?ÈóÕi˜9@%~`ÔV.À9é©óƒð»À<	‰±Å	Š@Ä{MSDö@SZðç^?ÀHjýÏÏ?±–c?{§'?ôúkÖ证@	€ãäky÷¿Ø´ªagùä¿ê–à·e\{¿à'mb*W¿à,&Ïw¢¿Ý:¤OÜ¿è‰52ç³ÙAGNbll3FGL J1829.8+1328MG1 J183001+1323?ïutããºd?‹,A¢Ï¯ˆ?KÊ£tT.?Aè9Ìڝ?sgèpÞ?Š¸0Mr/%?îë·éˆÉÀ?¦ñI÷è0…?H²‰†âi"?ZÁ«)Ñü? á·AWÚR?¦µ»ÌØ>ß?î4
ï›jq?'à|ÝFÇ?uR—¦¥9?g¬"÷œˆ?ª–³T"H?'¬-ëpWS?îJێ€ß?ŒýÔ ¼^?gWÿÁÚ¿¡?Qù¬O
×?¬ÕÒJúEö?ŒSË4æ4FGL J1830.1+0617?'OÙ£G1á@Wáá1àÀ9<•ÃKCËÀ;‹PMö-@qV…sÈ@Ž£yè#?¸´¸ƒê…Å?·ÎFO?ü#ûØSÍ@z$n?ïÒjeÏg²¿Útî¿eÛý¿äÎ×ؙŠ¿âHŠèü®<¿êÒûºöás¿ÜÉÇÿÞrAGNfsrq3FGL J1830.1+0617TXS 1827+062?îAp²g? lƒ`hØ?\¬/ègÁ?VÇG&"÷?«"_\;? 8ñû` ?îÛeG½L.?ªÒIëøC?JÙsĜºr?kRðûå?¡ÞEµÊ=?ª˜Û¶V?ëי²?¡îƒ^'Ä?"ë׬T±?‡†ÌC"k?¼Au÷Z¢?Ÿ_ÒøÿÂ?'=æ±?u¤PlÕï?Ll˜.ÉQ?>ç"–(í?‰N'ðSg_?uNá4hW4FGL J1830.2-4443¿É¢¯,}âYÀ.jÞe{"ÜÀ9BW@X¶À;é·B÷ÌU@'²^Ø(@L~ä­³?³XÚ©¯;?ͨœkÛñ-@Ú:_w^Ü@íÇBŸ6ç¿É6$ª.gG¿àG¯â0aG¿è¥ú?÷'Ç¿èeÞfRD¿í`b@fø¿ðAGNbcu3FGL J1830.0-4439PMN J1830-4441?ï8ƒãGTÊ?'™y"1UÂ?'ðwX=ó ?‹h#æû¸i?{ü0û]Ï?y›â 
ð1?ïÐ÷dzwd?~¡
~r"?3}X"qæÑ?J=´)b?vLF¤/š?}'3ç4$?ìñrõ/X?£Sd°•±ž?¦mҒæS?™\ÄËJ'û?ª{¾Ú|!?–gµÁN‰?ïÒ
ð$õ?ab>GÆ®?KšÚ?=ÕUôIÅ?sˆ‡­à©þ?_l¥C{kz4FGL J1830.7-2713?ïúÂå~…¨À"jP
_À9—ìoîÀ;¨uÕo3@nƒGr°@b¢§_U?º¶ñ™4ïÌ?¼Ö€TÏG@<h€òÙ§@u•ßû¨­?ïŋZ;µ¹¿áýwå?¿áýÖ?<Uò¿ÞÊÒ É¤#¿åÈ¿nÀR¿ïþ؃ªDAGNbcu3FGL J1831.0-2714PMN J1831-2714?ë¬*x‹ìâ?±°ÏÙ°R?9l ¸á?zš`?܍î?À=â‡@ê?°?wnÍ#?àŸ³Á;Kœ?ËYPoˆ'?ŸTAÍ£Û+?§"×µ?ÜËT`¯+?ËEM¨§þ?æ+éeN?«<Œ'ϼO?¥fVÅ!?Ž4ÐþВ?ÐýBu+(?¨ÈŒjsd?ä)-åçr?¤$LkYÀ<?¸Õýîz?—B1/[Ֆ?Ñwœtµ}?¡>×ÁÖº4FGL J1831.9+3820¿è¨éj‰®@4š€If{À;Pz9'ÍÀ<¾Ýšzj)@ cnv*S¼?þ†Ôš÷g«?ÐFðù²?Ð2?"?ý,©@։å@'ԱÿîÂë'D"X¿ëöòoô"¢?ïþž¦ž»¿àԄ¡ºÐK¿è"PïܜN?˜bãz
b>AGNbll1RXS J183202.2+382132?îý:ÔÕ«w?"fíñ?sÝòdÁQº?pž*\Ù3?›a(Ì<à?'~B°níg?îz`›²A?£Ë–÷ÔV?uíƒ}Ə?‡þ´ûµKÇ?¥œEÕ%¸(? ÝŒ'05Ë?ìɟŒ)¸Ø?Ÿ@Öw|Üä?',`þÇ?ƒû‹¨Ðû?µgë_r€?šŸT€?Õ?íS#J¶?ðØ7'÷?|¤œj;áã?w§bRA±?¶+0Aì&?´nY7cË4FGL J1832.6-5658?à"]âM+qÀ4m?ž{À9d8F˜jÅÀ<"a+"@qƒ¯½@"+¶g/º?±œÅžbe?®±±à¯¥?ú*M`Ûâê@ÙFœF?ì.¾¯R¾¿åt…
›¿à4º-ô¿àP"AÉN¿å<YjÕa¿ähÁTɅðAGNbll3FGL J1832.4-5659PMN J1832-5659?ïU°Ë¥?†Xf[G?að‹Ú0?U6¸˜úï?"ëÁ'åi?"ՆƝ$?ï[n™¿è?''LêÁrë?XXiµÆhØ?f@ä}3Ù?"·Ñkœ'?þBê½_?îyé\V5ï?_&\Hhë?v+žžTú_?g| Úý(ñ?¥›öfÒÁ?Ž5üö«¬ï?íËMN–¡?d½iÃz?"s²‡'ÇÝ?yKF–¿'"?©!çM²?ŠÞSáÒ0Ù4FGL J1833.6-2103?íyÔñUæÀѹ_1¾¿À6`°Å/JÀ:‰"ªNô@¸£Äë¬â@¦v§&J?‹­IòèÔ?¸eúéHÙ@&¬`gHäu@Aóâee¿Êg>ÀZ#¿ãÀVgâ¿çlë¯#¿ç%¼R+F¿ê>ùºì¿îö÷ãÑÌAGNFSRQ3FGL J1833.6-2103PKS 1830-211?íúOßâͦ?§1Îm<Ž?z1¢hØC?yÿšdÕH?­Í´¸"R?¦:òZɧh?ë›?‰rd!?Ç;Õf–*?‰)à_S?ŸÆbæÇ°b?ÀcØ`u¦?Æk&î&?ëe2Çô¤?ªV¤ï'›'?¥ÀnK©S?šìЀÒg?¹ö2¡£Ú»?¦Cú=(?îyÜÄh,?™ºJÅ6/?…9û!½?~"¬ú%5d?£´õ¶˜S?–ÚÐÛ]°4FGL J1834.2+3136¿ìOp2ÂõÞ@13¬)ÜrÀ:˜T+
pÀ<MAî·Ù @!6âågù9?þEäæŸê?ÌüŒ¥ä?²{;4´g¦?çu *­R´@ç™ZÚl?ïêõ6¿åŽü¢}mê¿ì›'û? \¸<ÇÜx¿ÝmmVD°3¿åÛBöAGNfsrq4C +31.51?ìÖÜï{i?¯‹_˜~?dn
N~iÙ?YÖå·ïR?¸¥¨0 1i?¯B'Ê…?‹?í_̬2¿(?¶»Žþäl)?xŒ:ç?ƒ:¡ç=?³xÙ*»•y?¶4áòýÆþ?ìk«<FÅõ?^¡"í;?€Ôd³e6Ž?oc´Þ¥L?ºˆ‡])"?›àI3þ?èé³X¨?«‰"{+?'íö·ìŽ6?†¿®—#oå?ÊtüÁ›?«~®¿Û¾4FGL J1834.7-5858¿ï‹¹wŽ	¡À4ñoiÀ:›ËáªÀ<6h¯ìÂ6@¬Bè2@'V¡ÍDÂ?Ð6Ö@hûÂ?И
M`Ûã?þV>J¾j3@	(#á≿ï_jÿR[?ïãyòÄ-¿åF;Šsâ¿ä&vVžrF¿îÚ"ö¥
¿ïþs£eË6AGNbllPKS 1830-589?ÊFâ?ٖNÙ—?nËãifkm?f¤"¡ÑçÜ?"¨Bs¬v?y»Vƒ
«Â?ï6£öHI?–ijeÄq*?`³ø.Ûæ?m…¥Æt?—û[z
?•,ö¹7l³?ìêåI¡?GŠ™~Ma?›i©¶GÐ?‹fK¢ùœß?±Îm!Ž?•k¯X{?í öܳ%\?–Á ùҊ?Šhlý$?vÛ<2§s?³«9,Ç4<?"ðFIIa.4FGL J1835.5+1349?í>X>ãô@#pxú½ àÀ:^qhøçÞÀ<´-™–?@xD6¿@M|Š•?ʪ < ð%?Ç­NWPôº?ÿw¶4ÚÓ @ðÓQÌ%ˆ¿ïÞf"‹=?ï˜j$aY¿ãB#%žõú¿ØÏ= ˜ò¿å/¼»Ý'@¿ïúDŸlArAGNbll3FGL J1835.4+1349TXS 1833+137?ìÝö H/Î?²Î¶½ó5?lÎ"5¨Ú'?j$N;ù5_?¸)Ýì:Ã?²•éD\?î£Oâ׋?ªðåf×/?]X_O·?l"0đw$?¤àKGYÎ?©û}Vµ5?ê$	ËÚµC?¨Þ»XÀö?'ó‰²ç?

", U?Å1gšQN?¥ÿPZ"7?í…ð)W?ê°L›P?†'mé'ÆÍ?qšK!àÛ?±öRîr?5Å<E4FGL J1836.4+3137¿èéWYë@0ÇQzF<À9ÃÈXÉűÀ;ã'‰±Å@·5ôƒ @ð%ï?¶‡Ü¾îy?žsÚÔ?å£|f'ì@	'tΉ‰?äPŽù,§(¿Ýùà4ì¿á)½h«»¿èŒö%‹«¿ã{6l£—I¿ÒS<}‰ÃŽAGNbll3FGL J1836.3+3137RX J1836.2+3136?ïf§k#ëx?ˆ4	N ?bÄaªò£ù?VþâQÒP)?Ò†f$<z?‡->_Cr™?ï@KC²ý?"™sÊê?VQ¯½½?bL-.TÇÕ?–'|—ä?"õ·ÌBˆ?î\¨=ÊK?Ñd™°Ðß?€æ(ÂG?tήàÐ?œ?¥ûñ÷cIQ?Lû·Áè-?í6ÊQˆâç?"#h65D?"¨	¢<?mŠ¸X:©)?³Æør"¡Q?'~Þâ=:4FGL J1836.5+1948?Þ$9¶3k@("'Ù±·žÀ:#GÃEeÀ<(¢¹ÓËÅ@tˆ$QC@ÖïÞIÌÓ?¼M3y…'?âmY09?ÓÌô9ù ?úJC*L.Ø¿ážf½¤:Ý¿æDw(U‰Ÿ¿ã F&Tþ_¿àËx¤V‹þ¿Þ╠Ž¿ã'¸ú‡ñAGNbcuNVSS J183632+195047?ì€wÎi!?®´Št0û?xLH%_d·?hi&ÊZö?¸g7¿6À¡?®Füç:??늛¥8è?Á¡‡ªŸœ?y&‹"C>ç?‡oT4Å/?Á]zCÊ?Á_å—f!?ëðøó~?¡äºD'X?~(n1âÎ?{…öj°x?¼ˆsZ)/±? R©û®R?ëëî¤Q?Ÿñ³ì«ý?"–\_7Q?€ŒÊôeÌJ?Áuˆp^Œr?ž¾Ý£Â
?4FGL J1837.0+5347?×bL£7b@7£¾ýq?À:"
xÀ<nCe°^@n]ST0@Ê:KUhè?µ'éÀè+迅Ln:Á?Í+éþ5ûe@æ åhã¿ÔŸ¯=æÜ¿èT×È©Qž¿çõšÀ[¥¿ãXˆAØg‹¿ë>"_¦XÅ¿ïÿ˒:)ÇAGNbcuNVSS J183710+534704?ïE‹÷¥–n?‹Pî?}T0Wæx?rÈXfL°?òéê§YP?†P=ch;?ï{^-¢i9?ô´¸Ì?Yƒõã3<?oŠ°zî4?ŽD©K¨?ŠŸ–i/?írý'2wM?™®âVˆa?'…
ææ:?†0/¿Èº?¯¢ien ?"«˜³}¾ú?ïDÇïù³h?{åÞâ÷a?"£"'Ë+?qå8r½Ø?Š*ánÈã?r¤HB–BØ4FGL J1837.3+1052¿ï-ÆH	•@ '5ø	'À9ÙúàŽµÀ;±Àn¹@gýY‡…Æ@b<ççÛ?ÕvŸC§ ?ÃQ]?ÌÐ?ÿºC'œüû@9C!ór?š¾\È¿Ýà鄓x¿ê/·éùr¿âu>`bì3¿çôñ^|¿ïÿûÎBÓAGNbcuNVSS J183713+105143?ïBH5R?¤ë°[*?g­I²­?e^z•K²?œsÇ
ş]?¤Ä´ã"5?éÈêxã \?Ãrõr0¤?wÈʟÁ_?‡?Áh?ÈÇss—?ÂûÊӌé?냌Ë-,*?¢¨¾TK€`?'
úÎRjH?:ΙMWÌ?¿ Úó?¡
¥ïbÒ*?êúUŸ)¹?›tó%f(?d¢'T¥û?s¶/zÅ>s? an¼?šF
Šä¥,4FGL J1837.4-1646¿è…g0ÂÀ9åâGˆUÀ9šsfÿéZÀ;úý9@.Û'X‰"@¾+Uï ?ÕOƒ3є?åAˆËëü=@R
Á‰¢¬@å?ïÞþ"v¿ÓtnÒE²'¿è<Ÿ9@>¿î¾£%¿ïÿÿ)@k*?ïøš°ðÎ4AGNbcu2MASS J18373301-1647530?ÉÙv½ö?Ã¥€·1'7?'zÊQ¯?"á€Òâ?éužz/;À?Ä_xÅÒ?Î1p¶í¿v?ÆW|GWù?¥l«a‰æ¬?¯$­<¹Ñ•?çÙ+ñ¸?Ç4å|n?ÐÜ7³F?­ÑB>0?Áû;ûH?Ÿ}SØ?㧧±K?¯{E5|a?É3QÊ4U8?¶•¾7é?©2ïO´4?Ÿa´m8?è ®}ïo?ºÑ¡ö!_4FGL J1838.0-5959¿çîiÞ§&À5¦¾zúr"À:®Èú°4çÀ<~PŽÌÝ@ ÀR¬u>p?ùÒk<Žüˆ?Ψ£!ؗÜ?Òw¬tg°é@ò¿-§Ù@¦žûn¿è›¤¡4˜Ž?î(ø|}ÿà?è7é{Y=¿ÖXF½ÿ}¿á\LœÄß¿åPŒ?>qAGNbll3FGL J1838.5-6006SUMSS J183806-600033?ï÷Û-?'%<ëAFä?q‹ñ\Þòí?h /%?
?›Z­b¢P?'»¸cY?ï(×BV'?˜Eu|¸¿?a²õxÜ?p-lK'Õ¡?˜®ÖöŒþt?•úJ¶"¹?ìûŽn
Ü®?œÑ
ûmÍ?é<k‹ª?ÊÙH8/?´@v7¥?˜"æ(xÝO?í(ÄÖJï?œ
ÔÃøF?'ä-‰Š¸?zã(ô=?´]Yhht?›#֚
l¼4FGL J1838.4-6023¿Ûk]œoÄÀ5Î/ßÁœÀ;Â~•1UÀ<™7¨ùä@!aéÆ,ʎ?ý¹Y_ç?ǐÈû"?–†¾(LØÔ?Ñcº¥@·ä$\V?ïå$|·
Ä¿ä¤ßßÏ^¿åOV_2?˜¿ÖE@[º»Ó¿æêNˆ#O¿·ø'wAGNbll2MASS J18382063-6025224?ï§*ã۞'?{fá~6rÑ?3_ÄI|Ÿz?'ÎĒ>?…šHæÌv?{´ë%<ô?ïP&¹cth?˜|#T²·?Hëz`š³?Z­¦«AÄÑ?•3Í'n?—Ö©&҈t?îUúÄzÿl?'¡Ký÷Å?`èLù¯ßÂ?LW7ÂW?©'ÎèµO?'FÜG%«ê?í»Ê¢Ñ´?˜¢êèZ?gx'§=p‹?\-'Å?±eæT=æå?˜ƒnï+ˆo4FGL J1838.8+4802?"|My°í@5҉üm¤HÀ8Y…O_¹¤À;'*è´@¿õ=Ú+/?ü9"ù÷¨?¡Dª©â< ?§Í?¹Ss@¢ÁE°
y@#3d1¿ÓbÛ, Å¿Õà¢A³Õ¿à-n}ŒÙ¿ÔhrÛâ`¿à¡u0.¿ÚÍÒ»ú²AGNbll3FGL J1838.8+4802GB6 J1838+4802?ïì'y»Šò?[™ªÚ½*9?$Ä(}—'+?§Hû<å?b"C¼›–<?[‹nŠA?ï¶ðmì8?ŽhñÆì?A5ìË	$Y?R\j-—o?f%Ô_£?Ž­¶"Y?ïÁåV¶¾?g"è.·›?qMa9Ì?f×KK%y}?› ¯üÚæ´?Šû(cÄö°?ïÚîÜ$š?_jÜÀìe+?&)œìÙ£1?¬b™Å!u?q×EL1L?__Êt]4FGL J1838.9-3457¿Ñ¬®·qÀ)—¬>·Ë´À:NÒàD²À<DÀ:î˜@#ݤ
‹Ê@®È b?Ä	çƒÝ?ßa¯²à'|@Ž6Kìg@ðÜvü?ïø©"¹`?»-(­Z¿áÌHþv"¿çà,€f—º¿ï¦tÞÏ-пï­ðÔ+AGNbcuAT20G J183923-345348?Â0OkÌûN?¶Sþ昆?äᢞ€¼?Å'ãdm2G?ÊI&0r?¾ÿ"0l»x?ן‰n@?ÈDS Há¨?Ý_¼ô9-D?ÊÓÖ.ª†©?Æsä±pù?¼W@QšL?Ðã‡wç?²xYmÚ2™?à×Øù*u?µÏpϵ¼è?ÊÝo+ˆ?©Ê)GÇ?×#™'ōî?ªqÂU,Îf?ÙÕÚl'6Í?¯ÄçÎ×VJ?Î
"&v‡?¤±œDøù4FGL J1839.6-7107¿ïŽ¾Oœ.À8ŸØ­«ŸVÀ:ƒñ'¨4À<l'ÐR@&ò	GQx@a<á1ޟ?Â6‡»öÁ?Ño^|âÿ"@ƒ)›üå@J肊ßB?Ð%óD/Ú¹¿æ*#ŸÂR ¿ê܍YýL¿ì\e'TPº¿ð?ïÿÖ°cAGNfsrqPKS 1831-711?ïêÄ(QÕÑ?ea†p_™j?UŸ5Ûh'?VG` ÿ°?TØzTxö‡?[?oŝ?ïEZ:~7?¡v¢X¯æ?kejúc!†?ƒbl´Æ?™*§YcÔ×?÷´ÅüÎ?ìäîJÀB<?Ÿc–¦ó!F? JxYJÎu?ÅUF×t?°³Q}X†Ü?–¶þ¯ñÃb?ïW®/Dè?€¯qÙ'.?cˆSÕë^?U¨ƒFrß?'™/´h?å?}øV§N‰4FGL J1840.6-5545?êÌÙYøïÀÀ4²ôàM/À:"µÄr‹8À<95>»@N©•·b@i¦Âwu?ÌF³Ã'dÂ?Îå=F‡xÛ?þ{ƒ@GþЪýÅ¿¡1=ßoοÚ]7þôè¿êßß~€8 ¿à‰T!ÀD(¿ïþ_–}Û?ïÓä^
ýDAGNbcuPMN J1841-5544?ïòÆÛNü@?bps'$ç?Aõ˲"?DO±bnVX?Qwc‰w?^Xkó͝?ïÈUH|`a?"SÔzô¿Í?9—ÿÞ«¾¶?ZêPR¨†?z;ÛÃå«?ƒ–Ìj€*?î(äÞó©?";:wžs?‰Ëy¡†m?ŽC‹[Õ?¦þðXcÌ?kÝö'¥"?ïí›Gº$0?Rv'§n)?öî·ÕÛ?Ó(-ãÙÔ?amÕ~¢?R ¤Œ4FGL J1841.0+6115¿ï¾¯¸"Ü@8ÉzÝð,À:+ª¨µ–À<"˜8p‰Ö@­Z—@iøÂ!?¶e Ÿa¿"HóÜ'«?Üùm'e™@šš?íˆZ吿çs×¾}J¿ë%§>Ê¿Òft©H›¿ê|•aütZ¿é‰@»±òVAGNbcu3FGL J1840.5+611687GB 184000.4+611120?ïÔC·×8?q§À~⺻?Y	Ç7nQ?R¾*2¥º??o<D‹?máƒEÚÞ?ï·ö}+¥?ÉхêB?@ŠëZùŽ?QÉ­ü¾F?ñÿgq?Ì»Få<°?îՈ~­Aô?ˆú§Ù]ӝ?uËý:àOm?nnžEêÝ?ŸÛð۟­¯?†LîɎ¶9?ï•Â1 
?q]TϺ:º?c8%!Ʋ?SÂýo£âÙ?…ÁjWôFü?n~9D	¡4FGL J1841.3+2909¿Óg°Òµù@-±«ŸU›=À:Vî#^ªÀ<)Æ°Sƒ@!ÏYè~¯?ùP¬:†
Ì?Äd?D¹mt?ÃÄ©Ü¡V@nÊhn~c@ØíÙ6èt?îæ{_ïJ¿è±Š¼‡l¿Õ"!'—ô~¿Ó«é]&KÄ¿ÁƒZèÙÉ¿ãúM~caAGNbll3FGL J1841.2+2910MG3 J184126+2910?äÓW™ýÔ?ɄŸ[)¥?v¶
;Hl?Œ×JÑFs-?ÕRwð(OÒ?É¿"UœœÕ?éùæ3?ø?Çé3đG½?—Ë_m}p?©ÆgD,?Ȓ¬yƒq?ÆzPÕf'è?ê˜W9ñݱ?¥ÝÁ«¥_"?'­3яh?…ÚdéÉ#?ÃI1¾WO?£×‹­ÏèÚ?ã.$¬¾Æì?«¼à@åÈ?–¨7ü(Wã?‰De›M?Ø93&¿ì©?¬[{¸˜n4FGL J1841.8+3218?ËwÑþdõM@/ô(²¦°ÙÀ:&jö±À<'-Z¬@ h–=º6?øå'Á(?È-Š½2Ðã?ϓºÝa @ËýÝï@
¹é¹S?ï×O!¦Bõ¿ ´T0ý¿â4»ÉoJ;¿£\|$56¿ÙÕÁ½ú÷Ø¿êÒ]«AGNbll3FGL J1841.7+3218RX J1841.7+3218?îølǝýÒ?˜¿±oÜQ?r'8DE?l¸r~³+?œQáþ/4˜?——e8{?ïŽÝýƒ¸¥?n$!²C?I
»V›?Wîh9©'‡?Š·Ôí,lû?¦¾Ö ¿?ë¨Ûm輤?¤Î@ØF$? ,¹7Fç?'|ut-%
?º¢Èwo? ¹KÛv\L?î0ï*V¦D?"ð¦ª?kY'ÛNÖ­?`†šmªçV?«;t<à®M?'ÇôËtÔ±4FGL J1842.3+6810¿Ú&É "'Û@9à(=5ëtÀ:5óÚó×À<FõÉEXÐ@"ø4.°Ã@.d"Õ?¾§à?†d?³?ÐÿŒh?ñ{½•ø$i@ëóbål?å}>" 
Q¿à²ù¢í]¿çýªðÙòO¿çV²X­@¿åÿ~?ËòÝ¿ïý:ˆ'
YAGNfsrq3FGL J1842.8+6810S4 1842+68?ï¢,ÄqÍ?~ۋ:àl?eÓîBX7B?^ÚmãŸ+?'þM~à?z-]'5â³?ï`vѱa?Œ¤|kÅä?X¬Ý×j?bÒޖ9¯?'p»X¶n?Štèf¸<×?ï,ö¤Ðl?=)H?¿?pœ®
?YÙý-±âS?š™º$:KB?܏>þ)?îˆZ—í#?'ËsÝubt?‰ÜLøÿI?o‹¸ÞŒv¦?¡CQqF?UkdÕ·t4FGL J1842.4-5840¿æY—$c%ƒÀ5Í!…Æ~À:'FÙÙ$ÊÀ<kÕW2@!ßX6øº'?ùµ>U¦$Â?À¹e¼ÈGØ?³ÒÈ ~vd?õÂäßJ@c?cÃ÷¿ïv³…Óé÷?î϶¡'6y?¥'@"ɝ\¿Òëý?Ò¿à±6¤û©¿ÇNògHºAGNbll3FGL J1842.3-58411RXS J184230.6-584202?ïî»5Z?Y¾…LßÂ
?¥Ú›ê;?(')d‰¡?`üõƒ*?YE"]ÌÇ?ïÊHc7ŒÍ?€…ïþÐÚØ?*ù¿q(?Iœd`u?z6œ3Õ?¦êß4²7?îWߜ9ܽ?™C¦Ÿç‹?aK}½#?X¡¥Ÿÿo?©mU"†b?™?EyD‹?ïi0{ûÉ?wŠ‰.úŠ?H•Çèê.?:OVýaèA?'BP¹6'?wH¨Ä×Ìd4FGL J1842.4+7613?éŠ*M'ó[@:ўùTëÀ:þ•{&çËÀ<zŒç¯¸@ߖK±YT@õ"yŸ(O?ųoC.ÓÓ¿±pþöÌ%?ꖝ^Ë@ÐÕ¹ÛX?âTO­¿ç`|wIãy¿èHèÜÍËпæ¸þ˜¡Í¿ÖÎ9Ì¿ïúµ¾=gêAGNbcuNVSS J184225+761046?ïÄTŸÝ‡b?yå™9ß'ç?rÙցðçü?v	Úå•Ïú?e÷³–Í[?f²ˆlãJ?ïŽ`
}÷¸?‰ºõø1)?Pï©ÆÄH?h›€ÊtÉ?ŠJg©‰H?‡WæzE=?îBšÛÎö/?ÔãÑõ*?w¦_–1è¤?gTk¨\a®?¨á†PJ_î?•"y?ï³»éS'?n•tI[qr?R(è =l°?J]â\T?€Ëè—2.?kãQWdÖ.4FGL J1843.4-4835¿®ÜdÍ¢KÀ2Ág#$È6À;#jJ µ'À<"Þ·°ÛÕ@ /(Œ't?ÿŠ"¢Óä?ÌGOŸÐjf?²ÐË_ƒQ?꤫`kz¢?ù!¥AB•?î"þ×áÓÅ?ï™G™ò"í¿Ô'd=AT¿éÈ»ÆKç?ÊSk¢ep¿ðAGNrdgPKS 1839-48?ï†âk'7û?	Èt?K:¨ЈÇ?Kf¦[¿ºË?Œ"ºž4ø¥?`ô¡uõê?îùܨëé?¢-Qˆ(dP?cæ«•ûW?soX6P?žG©©oÃ~?¡œŠ—Í`ï?í¡V¿-ʸ?'Ü¿ª9ãã?'†#O5uÁ?wûçN(5?°¤…œªû€?ó<1¸0?ì±[",ø¸?¤;]êÇ?}JÛ±Z…?|Ér«|?¸ y3dž?£!ÇâËÏ4FGL J1843.8-2011?¿:Ë`™¦ÀЃn—À:§\ŠD'À<\W=Ôvå@Þ^eþj@Ðg¤T?ÎÁ#vQÁ?â":Re@ÚÙºñØö@ÑË«`?ïÿ΁ز´¿È=䧉ò2¿´l¶!9¶…¿á[ā¤°N¿îɟ†B¤À¿ïôÒÛÇ5AGNbcuNVSS J184339-200606?ËKx®ÚP@?»l›ðjW?¨~È'±?¹¯!šÁA?äƒ"FG"?ÁëŽBŠÉ?ÑYÔ»zo?ÆȦÒ?»¦pêŸS'?¹¯ <):æ?ãÞG×ÎXX?ȤjŒQÄ?Þ£Vgõ?´È03žóÝ?ÑMW
0<?³¢‰¨#2?ÐH\"Ú³?§Õó;€?àßbØOV-?¬gÌ8~N?'ý\nJ?©Ú¿pGŒª?Ð⻡*K?¦Îå—t"t4FGL J1844.4+1547¿æhn ‰@!DqæÍ)À8¢Ž`€sXÀ;[vý^ù@ó%~¿£™?ÿªúêí?ªÿö3á?¸¼¨½Mþ¼@/½jY:.@£‰Ê™–¿?ïæ(S`'¿âzŒŽ\¿Ù8i}òõ¿Ýx6zæP¿äXÅÉ£M¿âØ€_5ðAGNbll3FGL J1844.3+1547NVSS J184425+154646?ï:NÂBŽ>?œbÕòˆÜ?MÚdœØòr?P²ÇE<…?—ÇT'Çp¨?›•§eÍÁv?í7î|…i?»©¹X¹.É?bÀv¹Ó
Ò?të@@rÕ?³p<ÖM<C?»pâ×Ôb?í:
F"Ö<?3!|?…†3\0¶Q?{,QãN•×?³~ç`S7S?š³iÃL-¡?ë/숊­O? Ç_×G?†D§`ð?mßÖ¼k6?ÁÜó_AÂ? |IiZ)4FGL J1844.8-3248¿éõô–WÀ*)#å¸VÀ:ßT¦Ë±À<VÛÉ¿Ò@ çk $|?ýƒqÚ7ï[?ÌBûRFI?ÁJ¬ ¯Íã?÷<c'í"Ó@¸c3V?ÝØ̵O؅?Ù›ÍÀ"?ï&;Óë¤ÿ¿ÔÐ{)Ðß¿ÜöØ9™…¿ç>¢ÉAGNbcuNVSS J184445-324641?î>@º?¢K(&û?`Ò¼¾ô×M?Y&&þ"A?®òÀ¦?¡Ð…/½Ù?îÖãrkLw?¨ºg×Ԗñ?aì–ί¿?'Í~±…P?¡€:ÞM•?§åÚ« TÐ?í/ƒþAÒ?—s4pë&ˆ?zzpîi}?gø‰¸Yoå?´ã0Hÿ
Î?–dÛ̏YF?êú¶é¢ÁA?¬%ܖ}d?†'I¤º;Ò?'òÕAÇó?«ÿ¿)W>?«ØcÅvÈ4FGL J1844.9+5709?ÔþD]@ç–@7`ÿ—$tTÀ9æèˆêõ­À<pOŠL@ŸÍ¾G[@h§¤WÚ?´Jßø"»í?¦³À¿Ö͵?ñ"wXüñX?û`gô°ì¿æX¨mqób¿ÜÀff²g¿äiÿöÅÅ¿à⣘öÜk¿ãö"¡¸!¿èÖNUÎAGNbll3FGL J1844.1+5709TXS 1843+571?•Öõõ?")G}þ?s0aJa?e…²-=¶T?¡Ã€ ¤w_?'àk?î—,'3Ê?§QSp§?‹ˆ9sњ?"HE8?©#«(Îø?¡›Ë Î±?ì܋­tÀ€?œJ½ÀÖb?',®V+Ê¢?'SHêÄ?´vþÏ	M?—û¡ Ò–-?ìm‹
sT?˜ß'nI?«q2°1ë?"p ¡ž¾?®Ý|x˜ã?'È,°zâ
4FGL J1845.0+1613¿íúš<§:@!cåÙä"À9Ñ°C)J|À;‰ôRLÓî@+³Ö0Ϊ@ïsÚZT?Àñ®X˜r}?§;ýå§?é^«QR+@ç;2±A¿ïü+ഐ?ïû4SÄ£3¿èe­¤™`¿åøç¨eݿᆌáû2;¿â‡¹1åUZAGNbcu87GB 184225.9+161105?â ¹[Ò÷?Ã^$'û¢?' rÿЪ?‹¾üK*µÒ?ÚѽÆ]?ÃXÄãÓ®X?ê–/ºX\?Ä@$ü?'cÏÌ-?'™ê/Áÿ?ć
 ÛÁ?ÃréÄ?Üu›X÷ï?±LL¯úNŸ?¯
_H‡ÀF?'ì£-:ç¤?ߨ¸ø–	?°•3o:Ÿ?æäN¤»£ø?©bRŠÁùV?œÞÂå??"Œë}Pè3?Ðuᜉ¼?¨Z7n+pÿ4FGL J1846.7+7238¿ï ¾#Å5@:%9C¬ÅÀ;r«¯EÓIÀ<õøٛi@!‡Ý^?{k?ó|tðlå?ßÀç,¬0?َޖxÓ?ÿ›x¦@ÿm[M-°?í[Ý¡[Z¿îñÄhz<Ý¿Ñç3À̹W?Ú¶ÁÚUv¿Î0¥å,j¿åÐîš|îhAGNbcuRX J1846.1+7237?ïZ1aߓH?"'}>]e?cÔØ1Ž?e}~£"(Ã?'?QI
ð×?')•!Œ.?ïr%/Ò/Î?"máó·a?R™vJÏ÷H?nHjA"ñŸ?'¡
ì?'MîÃ_¥?ìï_`1Äù?ŸÄ{ç¥{?»9ŸtSÐ?r"òð¦Á?¶‰Qdz"?žyJëCI6?ï9¸É!fQ?†<èص'?5-±ÈJÀã?<ºHcã!?˜t0²
Æ?† P©ÑN4FGL J1847.6+5219?ï¿T•>Ò4@5¶–6—lÀ:ñXeò£ À<¾ÿ
6º§@ljßgY+?ÿ̀CRe?Ðc"GÁ`?Ð	ZÝN@XCùTT@z$'±rÿ?ÛT9}¥Z¿á*¥Å÷Æv¿â&©ý¿ÞÓ¿àÐ×ôH;Ù¿é¦n£KÊ¿ïÿþÞ÷AGNbcuNVSS J184754+521513?ïðöæ+Î?'D'ž"uÇ?qÖWײÞ?içd¬Ràž?‡–Z›s?}ý½âz	?ïKÀ£¨£?'…Oôi?fy'bó›?që//†«4?™çc>>?ØöD\?í^p~O'Q?–(Êï¿ñ™?"|
âØ?…˜­Œc¦F?°-Xü»?0xs‰ï±?îpӚ¯5?†uŒ±cà¿?†]fUº' ?qn'=­"U?£[lÂvgû?"îZ14FGL J1848.1-4230¿¯Öâ«TƒÅÀ1_󾩛À:Sˆs©À<(ôB\›â@Ä:P]æe@‡zÛ?¿e')]œh?«$|a$ˆ ?îVužèŽ@ø`ÍöŸ?ïöðÂuZö?ÓÒ)-ó»¿é¡¿ØȄ¿á|×­O¿æEòèn¿ÕÏ°¬AGNbcu3FGL J1848.1-4230PMN J1848-4230?í¡¯Êù"?£]æj³ ?‰èô̒÷…?ƒ&¯Ž]?¯jÆB?¡…Z¨ˆ?îÑnñËf%?š,9ßßÖ?gßþ¶oÒ§?nCImØH¨?¡k÷â y?˜vhpâè?ì æËbÁÔ? ™SàÜè?'r•m»Ž?}ÙÐqÎ5?ºœ$I¨k?œXÀ÷ã!»?ëð?&Úà?"®×Ö4\Ž?Ÿ;
–«¾®?"'íñ("Ê?¸¯D#~+?·¶jLŸ×4FGL J1848.4+3217?æCò{»•Ë@-_r'Ä"BÀ8'ÞѲÛÀ;il«$@#åÓ©‹@B[úҙ•?®(~îÙ£?Ç5Z«'@ó<£~@ŠÂ'4›¿ã'—|ˆç›¿Ùl`üD3·¿â¤«ã¢Ò¿ç皮l¿èʾ­	c¿ðAGNFSRQ3FGL J1848.4+3216B2 1846+32A?¢žµ?ŸÉ%úV«B?‰.Ë9¿¥?†á•…+±ã?ž«ÖæI‰?›ÕÙ› æ?ï¢W…-ó1?‰B‹•ÎÁ?NN6uº²?h§Ù^Ž²–?……;M'õ?‡rÑS1®?éš-¬3·?¬e«3½M?¶hkÉP?¢ƒÞ@=Çí?¼Æƒûù?£kLÔÆ?îÄYB^6u?Žéû,lhñ?\ÚåsþÐ?P÷ÏrŸñû?¢Ó"®|¢*?Žg"Ë'Y¤4FGL J1848.5+6537¿²ªÖ©€¨˜@8Õã§Ú¤ýÀ;1CºióºÀ<Ú!›[:¹@!'³­Áð?øçKƒŒ?Î2Sº<Qj?ÆÈdȬ©?ûõÓ £äv@ö{¬ô•>¿çW>«6z¿í²1«s¶±¿Ì"Æv)¿Á!JÓbé¿Üà4óý">¿Áº†ú¾VAGNbllNVSS J184822+653702?ïvç«Õ·‡?"ý¹´
SÅ?P•Ùmƞ?QôØ7×?¹Ç²2º?"•­q?ïŒÒM¹¨?ˆsiUù ?@~±ÿä?O(äœÚ6?‹Ãžqž?‡à(Q¡îF?íêê¾*%?˜ñý›Ýʄ?gÿ­€G
ƒ?W'"›e"?¯ß¶|í?˜¡GCɛ¬?ï!5tK?'aÿ€D?HDW˜U??)(aŠg?›6"«Nj?'K+±ù4FGL J1848.5+3243?íÍíc¿'@-¦¥.ùÏÀ8oSö!YíÀ;®»iÎ@hé‡B©ô@ß=?%°?¨iäöd?º˜»Î!á|@`ÔV.@¨ê×ÿ?ÝN;Í5¨¿ã9€hÆ¿æ‡Íôêù¿å';C¢ìÿ¿èÐÀ⳾߿ïþ¶ôô3CAGNfsrq2FGL J1848.6+3241B2 1846+32B?ïšÓ¾GË}?‰õÙÔ_½?feK¿?'¼?dù†
?ƒ±½~=Vz?ˆÎc.¼<
?流Ú1i=?‡×Ç*	ú•?Mxî7";?_‹Œ'œgü?ƒ'}8Â8¼?†Ö40¯?ìƺ5¶î?£Ìu~@/'?œufUòœ!?bW:Ó?²¬Ô¼Ëè=?¡st@™Š?îÓ¯"P'ì?‹So¿Í?kZXš—¯?[<ùÚ»Õ?¡e¥m7®?Šh·0`]ö4FGL J1848.6-2711¿ÎRì3MÀ&é§~^ª°À9éà¸<À;¹á`x@_ß4ÿ@S{š«'?ÊÀ	šÞ?ÓÈ5Ä+m@OÀ1³×@ÂMò§'¿Ì"ö%j¿â¼è‹+B¿è±`Ëò¥¿êétšпïþظ"Yä¿î…§ß­z!AGNbcuPMN J1848-2718?æÄ¿v·#?Ä]û'ü?£™¹ã‡ŠÉ?žõsÞÝ]«?ÐJ¼¡ c?ÃÀ\ù'"z?䵌Õbœ¡?Ì»Ò÷?ªÏÜùÍÁ?¯$z9¼•?Ó;¹›?ËôûöÅïÓ?àÈÍ;øë'?²¡ÄKù ±?¾Ô+ÆrE"?Ü÷eŽc?Ö¹Z–q—w?°3­¿`q?䮧®ÀX?¬€±"Üå?±v³àyIè?"B¬äè"?ÒEȄ,Ø?ªèΓb±Ñ4FGL J1848.9+4247¿ïÿ¤cÞ2@2wiDg8À:"~ù˜À<…uôxãA@ 2N@CRë__?ºÜdÅQƒU¿{^^ÞßS?½õc|@ê#sw›î¿ï꽟ˆF?ïÿ–þߙƒ¿à&D7guZ¿â0"!'÷¿¿Ü6^`Þg)¿ÔÄʟËãAGNbll3FGL J1848.9+4247RGB J1848+427?ï½®5ü?ª–±p«"?M>
í€?J'ÛÏë?}€ðcÁÝ?M/¨8?ï­E]Ù?"06'@?@ôªsŒ™?R'ÓkÙç?ƒŸq†'‡~?ƒx"48ã?ê¤;?‹eÞ±ÏzB?sŸÄ"ø¸õ?kÌïAL?¥qˆÃ7•?‰³GùeJ?ï</>W̽?{»ð¶«¿?k©ý…œQß?YÏ^%F?•؄RÝþ?zëZ&"Á4FGL J1849.2-1647?Ø«®@çôÀdkA—zÀ9Ä/µÐ1À;áRƒZ'ô@! •ÀR–?ÿ³LØç?³Óc"ÏÛJ¿¡t=‹Yn?猪Œžß?Ø0=³Gs:?ïЍa'^¿»YÓ0C)¿åè°;Ä|¿à¿…òèn¿Ø=ÏCtžã¿ËpÀ•ÆAGNbcu3FGL J1849.3-16451RXS J184919.7-164726?âÀîg}Ö ?Ãõ:úµÒ?…Yqíâ©?'–0‰¶?ÙÓW¨Dä«?àP›Äh?ÉDp^an?Èŏ#!?­•_¡y:‡?¸ÏŸrÒê?çՍîP*<?Ƚ8`ÿ~¬?æžßé<6?ª 0H¼¸:?šk¼Üû ?ƒwÒÎø†?Ñ"d‰Ã?¨»ŠÈ"?NJ{´ˆ?W?§²"%!?ÊYir?µôvÿ?ã‡OÜÎ?¶Uu=K¦ý4FGL J1849.2+6705¿ïØÙ÷òY=@9
ǸÕ¦À7×Øã["‹À;"1ί%@mvK½Ä@Äù¯"?"œÃ"\©Ø?¸'t·7_@""ÇSçá@EŽŠ$¿Êƒ]Âþ¾¿à.ë¥Õçÿ¿ä»ð¶ù&¿äâ1ƒ/ÊÉ¿è	}WC´¿é%¥á¦x¥AGNFSRQ3FGL J1849.2+6705S4 1849+67?ï²>¯VQî?vVvJr?T—7װˉ?QƆI©±5?€Ým/uk1?tÒ½J&?ïFÙÚèß? ®r]äÕ?tnb³`ô?Œ'•é&'s?˜ÛŒ?¶Ú?šyÞî?îͽ*[Ï?"ŽÉ'J(?Hy=Ùbß?‹ƒ½äù+4?–¤ÇԊ?‰Ú
ÆÂç«?ïžTs3F?|4ÛQ™£?cxuU.Õð?_eHÂL?ƒŒÅÝâÇT?y‰–¥À4FGL J1849.3-6447¿ãøGÅ•ÏÀ8&A€ÓÏöÀ;+–^{¶À<¼…"êÔ@ æõ'çôp?ûyüE`\a?Ð˜'\?Ï||¨G1m@BؤU@wHÐöR?½ðÊ1u?ïãNÿl‡=¿åÊÁžpn¿»¼$^@|¿Úœ=£N¤(¿ïÿú Âî'AGNbcu1RXS J184924.8-644933?ï¥P>´Ï?|â&LŽœ?]ðWÒ Ð'?Tnt	™Ó?'íåXˆl?zwGÈúå»?îÏFš¥L?žWќókæ?lèG¤Û
 ?}\ÏZŒc?¡=äúo?›vœ"·N7?íÜ
ڟ?"W³Ì<bŒ?ƒû(Õàf?v(3ÿê?°'º|¦Ï?'sÜHLÀÖ?ì<Oø	? s	%ð?'ÿúêEC?‡lãÝó~?¹]…2Ž,?Ÿ#L¼W^4FGL J1849.4+2745?ѽZ*»6ð@)U'Í}åÀ9÷ö•3À<&/Ta"@^dŠ$\@¾‡Ó[?½pÛ	{~Ñ?ÀÀç¦ÂÌï@Ü \–ÙÌ@e£zîޚ¿à«Ç>B…â¿ÚC¦³]þ¿áô.`:¨H¿ç
áŒR3¿ä•îê.¿ë¬ížÔkýAGNbll3FGL J1849.5+2751MG2 J184929+2748?ïs);ú?Š¡ëXKÜi?f©²tP?bðG¬h¸?‹mŽÂ?ƒ9I3?ï{}ñ[õš?c¥ŸzRÒ?PÚánå ˆ?`©Ã—˜f?'{%õ*?Rµ"c»*?î"JåŽI?‹Ý•Dj>?|à<Q;Ž^?p}ªÅÑñ?£/Ww©¬?ˆLÜe=Ï?îÏpŽË÷?ª\!·xÙ?uÈÁúÃC?]$}Êç…? gýû7†?."‹ˆ\4FGL J1849.4-4313?às
Í·ÈÀ1ÛV†''À9BT^üå™À;Û[Z™ª@Ú`	]L@úéZ¢
?­	*ÃoxU?½[3­VÚ@Kèÿ2z§@¢ç÷ ?ïÿã°> Í¿ÙAf|·¿âÃ{_œÈ£¿âAb ß9¿é'´þyî¿ÑM`pƒÛAGNbll3FGL J1849.4-4312PMN J1849-4314?ï°4ñ
	Á?}?Ìì¼?a '£ÐÕî?bÿ¤¢"
?UF''´?wæyP@?ïy§c o?ã.óŸø¼?Z¬ð2‹¥"?hf9ªÀŸ??Žg8 æon?¹ë.`­?îvógn?"qK³r)?ŠO&
¬?"@4£+Y?¢=uÅU¾?‹.¢è͸/?íÞ¢Ú.G?‰Rq®Dr^?l<G˜?s–¶–¸‡$?ªÜÊΎ	¥?…¼GX¼34FGL J1850.1-0758?ë<»êý9|À
½œtÜÀ9£Y7©ºyÀ;p]j>b;@'"ß @!ñÂO›I?¹f¢vb¿Ÿ 6^êNÆ?æ§VPn­]@羊êª-?퓢¿]"›¿è^ï^Èt¿ç}1¦¿ó¿ä¯'Á8¿ã€!ß&¡¿'
©¥š»AGNbcuNVSS J185002-075842?Û"Ó(í)"?Àñ±ñ?´eíµ†¶?…çG·¼K?áïÄÓҕ?Á³'£žÖ?ÞS G™ ?ÅêÕc̏?j­þšä"?wî«ÃT£?ແ݃ÏV?ÅÝÉ Ý?Û/4 «'?±n¿ô'?¦¯Œ½š–?‰YÑ
Õ?àým=Ў?°‹gb7WŸ?䊮'å?©æÚ©´a]?'Žx0Ø­?~Sٓûf±?Ö¬ÜÓÌ­?©v‰/ÿ2\4FGL J1850.5+2631?îüµ}zÕ@'ÛeDþ6ÒÀ:¹ß[DÊ4À<bèn@"¾×M.\	?ú'ðßьO?ÄÃô÷cNY?«ˆã$8U?çF߂±öˆ@ªöŽ<C¿ì3q|D=?ïϤîar¿Õ—"{ªñ0¿ØGt^4¿¿Þ²qA`Èm¿Y7ÕÀwAGNbllNVSS J185023+263151?ï7S²kה?"",'ï"?L7L˜¢5J?G#ß±Ri?˜3ÏM¿û¾?"\RŸ›?쿐Šî#?À&¿ïjÍ?i[¿¸"?vž#Ð:‹?¹8£Ì	"?Àg.Fê?ì½yµ¿µ?ýÏ]šJ?~bb8Á?l@¹#Oê?¸.	[ã†@?œ X.¸G:?ë
Áϸe¹?¤Ï©÷l0U?·ç0É <?'›ÁEÕe?Á±ûÛE?¦#…eŸ¢4FGL J1851.5+3406?Ø@ýSÛÒØ@-šÀY!À:;ţàÀ<n}'Þ[@@+0Û?+@Ÿ¼?ÈU…2à'?¹'8©ê ?ïf='u^@vwŽ
?Мöÿn5¿ëäa>y¿šW'Yb¿èÅŸ,«…¿Øò»ÈB¤¿ïõ‰ŸP'ÀAGNbcuB2 1849+34?ê|‡Lcâ1?À)‰›#Œ0?_¹˜°	
?VpDÇ'>?ÅÎ][?*?À$¡ ‰@´?î츁ÅÍ?¢ƒ"à%…Ð?V¨Äjgfò?el­@ˇ? 1À\‡ñ?¢+ydCºÕ?í"Nø¨=…?™É—ÿoš?yÌf(d|ï?qp™‡üç@?²@ÁØ7Ì	?˜nÄèÎ|?îԓFav3?"Í"É
<?_fOëŽrÁ?QC<Üø1¡?¡»™Œ)'?"'çT)'L4FGL J1852.4+4856¿ïò)̓R>@3òÜ]cˆfÀ8ä
kùMÀ<+ÑÁÿq@±à<Á&{@ï"b*˜?£&b•K3?ª†·>Æm@à5z5PD@&NIºO¿½6‰©âg¿áŽ­½gÿï¿å§|æÛkÌ¿áõÁb¶Y¿å U—¿ìÝ5Мe&AGNfsrq3FGL J1852.4+4856S4 1851+48?ïÚvè
?pޙ‹¼0?7üEæ÷n?1'ŽÒù'?qs·fƒU?oY.T£–—?J"ä1?Û $}ÿ?C€—_~|?Z¤C]¢:?:¢¢'?€ÇØÚe—n?ï/]ârÜ?‰ôŽÖdv?m4«®Íâ?e‡à©Hô?™s'î;Ê´?ˆ½ü¨>ȏ?ïöÓ¤—r|?CôY ¿á=?+,˜N)?ƒ·»¾ ¯?MæGŽ«®3?B4¹6â=4FGL J1853.8+6714¿íç¥×¦«·@8£NÛʗÀ;@8
‡=À<OìTR@ z}l@($¹ó¬5?Ò¥Y€ÏÉ,?Çrç~(úË?óµZ¥hõ@‹ÒªÝ8Ö?Ò/£#Ü¿íheå7&Þ?Û5ÚØS>¿ÜóA«›ú¿ã€;ÄÒ,ˆ¿âùZ"¡UAGNbll1ES 1853+671?ét'†Ù!>?ÀÄvqñão?²–]™/Ç?‡}¤W{	?ÈR~Áè
?ÀN–¦à§ø?í´}3íîè?­SF¨¬‹ü?‡gçΆÌ?"4x´Q?®Þ2Í^Ž?§%€™Ô_?ì!;?èÀ?¡R1U]Ä?ŒMø¸w^¾?€!jŽî'r?»lfé«­?žÎë0–B?柹Ða?¯%F	w\£?†²ÿJh]?|¶SØÚ]?Ò
õÿŸV?®ñWðÏÜ·4FGL J1854.6-6007¿îÏePð;À7®Ý&·#îÀ:åùrGEÀ<¥¸	â@ù&
s±?ýâEîÑ?Ðd!s€?Ñ3©$Ññz?û¯É†Ç.þ@ÖQ·'¸­?înkón!¿ì·¹ª±?âP¤'ñ߬¿äqÎly¿àNQ!/Ð}¿ïþ\ÓAGNbll3FGL J1855.1-6008PMN J1854-6009?îâM•Æ4Æ?šëÌbær?h¼•cLfh?`tœÖ|Ùp? O]MgíK?™ó,Çe}T?î;§xÑw?¥ž~¤/~'?x¢ yŸ^?ƒ+Cm7ý?©1Dc´ªâ?£•übÉW˜?ìž$/øºQ?œïAʃN?">ۜI_-?ƒ
¸hë÷?µÿ'™'Õ¤?˜ZdF~Gò?ê›ø$ðj`?¨*–È?‹ç{*ìX?'¬wKÐ
Ý?ÃØô‹§¹?§•
ECAO4FGL J1855.8-2028¿è‰%µUÀ$<âó¾ýÀ:ÍËÕVJÀ<>¥}Ójv@8£ÆCEÐ?ü{"¤£?Ô%ߙX+?ÝÎÆâ}
G@¦ò¥¤i×@	%rÒ/6¿éŠ"XŸÔ?ä¸Q€%TM?î¾h›Œ¹¿ÐDHÄ¿ã¿éåBnºs¿ïüHOúêAGNbcuPMN J1855-2027?ì+×B-[f?½Ý+"/û~?€¥ŸÙgN¸?‰=WىôF?¼Œ'óh:ð?»×;ÐE»?ìÑ?ßèÕÇ?Ám×{¡Ò?gf|T
Ñ?…0rþ]æ?¸ºÍû:?ÀõÝÇÖý?é{ñ§?«/3*ï6?¤s)SõÇ?»•Àá*&?ÄóoþŠq?§x֋
j€?íýÅãåª?žÕ֚ªè?q¿¸wvú:?m˾Պ+?­ëªÀÒÆ?ž‡G*"äE4FGL J1857.9+0313c?ÙD*Ñ(ÀØ?$yςgÀ8€Ä0FéÀ9É瀭9Š@󾑠¦Ô@oÃzn?Ô¨(÷?ф(£ãž@	oŽÀøƒ4@ˆLôzeÍ?ïM›^•·¿ìMè@EÀT¿áÁcâþ¿çª.£ˆ0¿è°KŒÆL€¿á_#a.AAGNbcuLQAC 284+003<?¼'×ùf?€~yµi6?š¡¯WÿþË?¤óh¡ää?îä9àp?§9
ôïܞ?¥Ä¯ýçK?¦Ìt´bj?¢Òroev?¥ô¹&˜ðg?ívÙ+8l?±!Ã|q›?ºÐÃOûLÙ?~ÊqT?¿°Jž©?¡•JÅ?è¯ÞTìÁD?¦olRו?ˆ  "ãøG?v±Ô9¼~®?‹´nø'ã¤?{;¼±"Nf?ï.«ÁÏБ?ƒ=Ÿ
d]4FGL J1858.1-1821¿º¢LŠaDÀ#]FÞ	5À;¯¥t™/À<)ñTk'@ v‡¬‡2@
 >ÏH¨?ÌǺ.d—?–î$"æ°?Ð"g~>tZ?þ6ÍVWP?Õ_"¥Fv?ïÈ!‡¿¿èxpT%ò¿Ýùu3ܦ¿Ý¤çá%If¿åŽx¾­¥?AGNbcuNVSS J185806-182314?à>‰)ô©å?ĒýµRæ?sÇqø±?iR]úŠ,?ß3Ïä45p?Đ ³C5?ääjîeñ¨?Ɂò³s'?fаRT½?wÆP&~ô?Ö	ˆÃx?ÉlQHr$³?è׍Y7&j?ª
‰‹§%w?¿_¹
a?x~R+ÇX?ʉުìD­?¨@_Wû˜3?éțÃí·I?¤@ïC˜ï?Š¯íp'õ¥?~Š' ñ)ì?Ç2'?óƒ?¤—ܕ4FGL J1858.1+7318¿çØòr×@¢@9k©Ÿ¡—À:qt4…BÊÀ<{Tç4@ôœDCѼ@…w£¥Œ?²{"O…y¿¶lþ[EB@E–È.›@_ûé
¿áˆØÖ+¿ãMMüUy¿íMÖýÓ*	¿ÁÔüÇuC¿Ú{"BšY¿èê–o AGNbcu3FGL J1857.9+7319GALEXASC J185820.26+731714.3?î2,e¦N—?¦õIeÈ?'yÚͳ–?¢WÜ+®?£•|¸4<Ò?¢F
žî,?î½îOϔ$?­Ñ³C3"ó?çD•uº?›Sšø Ñÿ?Ÿ¸ÂcÂÀˆ?¢Knü?ì—ÿtªdV? ´8Di¬.?"8‹lp^H?Š•lô&¯"?¶1áÅ¾?œƒž:Rg?î"Ñ)ûÈ?•7ô›?y_ñÉ?†—ï íZ?¦k+#ý?êg[
'4FGL J1858.3-2511¿À/ÿ
À)6~À¨À9!áKßÒcÀ;§5Þ^s@ÈWC"?@µ»8OÓ?±¸põ5¡¢?ÉX"*ø&@e8}@6sšœ³?ïü··ïÆ¿ßÞT~ÝU±¿åN¾Ôçx¿ä!H2ž¹¿êª¡Ô¦‹¿ïÿCAž0AGNbcu3FGL J1858.4-2509PMN J1858-2511?îS'N_?¯h«š)U?™!£=L÷Ø?«Oߧ@›™?œ}J˜ç%‹?˜°1HT É?îïbÖX?¦-Ç "kù?tHÎFŸ|?"áðˆö?q«m?¤‹0ò:ö?ëºVÄ
% ?©V7õt'~?¯µµª? 0‡Å
?²^º"¼?ÀX¡SR?ëcfb9`?™Éf±~×?ŸÀìXŒ8 ?"ãËYýÞ?¼÷¶Ë&ù?–`ґ	{H4FGL J1858.3+4321¿×"zŸ>°@1>ž¡À:±Ðz×6³À<‡©qÛ@…z±!@›¹!]¹?ºH¦7Û?±¦ÿ!¢€ã?ïÁŠ¿66H@Ö%f
?í}Zi"?АC¯'9+¿èqÿ¡¶I¿ÛÔS±Wü¿ã€§û\,Q¿ïÿÿÊPËAGNbllNVSS J185813+432452?ïQ™Îñ˜?‰vI‰÷׍?pÐú2Ý؏?hºŠÿÃÍ?'˜‡•‰f?†>C‹ˆÓ?îUËæŒÉg?¨Y›nB?týç¼ÝðÞ?"ºÍü
d½?¨"Ÿ—«‰?¥ëµÑò‰?í"$îZ¦?"ß*"Þ`Þ?†ŸÆi|ü?s4¯§Tã?°¤¿û%?'b×(xWZ?ì¦ÀÙ
?"""ë$ô?¢;'Ôû?†ÌcðŒMÜ?±±–ñº?'m ^•¹4FGL J1858.5+0640¿Ù…ìFBb.?÷øZðŸÀ9›=EÀ:…õ|ï>è@ ºu\M‰@F49Ãp-?Àå13ûÛ¿EłVž@[?çK©!?Çæ{Ÿˆœ?înÊî¦;i¿ì.KlåÜ¿å
ÃþGB¿áqüfîK£¿á®M?ùÀ AGNbcuNVSS J185831+064016?¾uéEã?¹÷3
Æ?²'™rK?³6U= á:?éìO¼é"?ÂMóag?Í®r±…é?Ä7P=–?˜ç7•ñû?¥18š«ñ3?çÍBf«Võ?Ċ[%´p(? uçø?£Ð•[̞‹?´ÝÑîdtP?™ÏN#)hŒ?è¼(H5lp?¨Wa£¹"á?Æ2H¦Zܵ?«iøsڗë?–çÄÃw±=?ƒ'Äž+˜¢?é¼/°M‹I?¬A"Îы14FGL J1858.7+5708?è‰yL¶Ö°@5Ìÿ!³¯À:Æ÷–¤ò"À<¥¼ä!}(@ƒ¹ügÅ@ÉYø™Ú?DZ~è"Q×?ΫúÅ-œ@à f§ÔÆ@oüt°++?ïòæ§ieõ¿ÞF~1ß ¿âxP©e¿w¿Þµã¼¨gh¿ïñIï7Zà¿ìY? (ªAGNfsrq87GB 185759.9+570427?îç!o9æD?•Ã%E%Þ?†kò·'V?ƒ_Û
Á¿?—åؽ/Œ½?éöíú?î9û Oº?¥'ïá~?‡0I«Xš»?•á[³ª´?¦"3.9? «M™?ìp]«¤:?ž™ÀÓIh?¡®>TÛXÁ?'fãæÎɉ?³¥óxrÍ?""†òçÓ?ì‡àÄÓ©%?•ßDùŠË?¨ÃqÑ(y/?‹{vÑ?®¾áœôy?#Î4FGL J1859.0+2329¿À™-ý®@!ÉdobÀ:M¼àÆ~ÕÀ;á<aNÏ@F×zzÅn@ã `ȗ´?Á,C܄¿€fX¤†Ý?À§H®ÅzÉ@Õ;@ráÊ?ïÿŸR@>´¿ßqªgG7¿èí5" ¼8¿à¨>b'D¶¿á¡HÌ!¬¿Ý¤ëGWAGNbcuNVSS J185857+233007?âv\ÔÑ5?Ã鄝VÔ?xú)
??~-¯Xl®s?Ú'…®Œ‹+?Ãi±M?ÞíMÿU–?ÆÔ÷ã\?ƒ)…>Ä
Ö?Žm|›$9?à¥ãDDý?ƛA b+?äöc¥Å˜¼?°¥š4:ˆÇ?¡ÌÞ~Ï÷?‡³P¬Î¥?ÓٜäšÏ—?®ÇÖOñQC?é•Á âÕÝ?›ÜSü×Òú?Ø!c	²?vÝ¡kL¸µ?Ç«zÊ^wî?›ZnÁZ@Š4FGL J1901.7-5140?냗»·ÀeÀ6{þ;â
À;FÔánDÀ<µgÓMðN@nl <K
@è"úô'…?ÓÁi¢#?ãgþFÂ\@
0¡C§?ó ·?ïE´À¦Á¿×Ñ¡³CŽË¿Ñ¬ÿuìk¿äbÆÜ	¿íÇ4—ɶ¿ïó_2•AGNbcuPMN J1901-5138?åŠô‰mD?Á‹B©9?É*‰±®´?¾	ëgÀJ!?À©¤(œ:þ?´-,wTP?à:‡ò›-¬?Ó
Üô*y?ÕE€šb
?Òß³ûº7î?Ċá4^…4?½
Z9˜?⊽-‡\œ?²¶ð0(V'?Ës=i­Â¼?­áÍÞVÆú?ÊaÍà4ÊÓ?¨–ðÐSé?Æ`X?n?£¬¿1Á?àatCž?¹1»£óÌ?ԝ/wÁ½?·¾·2ˆÌ4FGL J1902.4-0629¿ïȨÀŒ°À‡â`²È?À:Î-À,«ZÀ<sY"ð@!¬Ê†?ÿ4«ˆ¯fŠ?ÇSŠI{õ?@àWt7?˜4éÊßb@%'}?ÚµŠ;Þ§¿æ w~瑟¿ëB1}Ñg?§­?·T¿âøô=Te¿Ñ¸#@¡ÜAGNbcuNVSS J190223-062850?á·8©Kì€?Å|B[¸ñ?o'T'«ò?ž¦Y…‰or?ÜRl;¨?ÅI(S¼?لfi€šˆ?ÅÆ^aÂFÜ?h«±6%?{LˆçÄê}?ã%!	§—?ŦÅ+ƾI?æXfu–q8?ªIÀïÀÉh?àF}KÆ?u3	«˜£?ÒA1@kHÕ?©LYXç^°?å2¥È^3Ä?³X"g[3r?"¿«j`_?zÏæøTœ?Ôô·òÅv?³l˜¤ö4FGL J1902.9-6748?àX¼SF½ÃÀ:$咖pÀ8ðÜùjº‰À;ù$(Ô4 @¥Tƒ™@¿æ4|ß?¦O§!wþ?ÀǃwCXo@*Y:-ù8@‡)ÜÈBy?¯åµüÑ¢J¿à›NÛ/f¿ç')oe©¿è.¨>Íñ¿æHp¡þ—ö¿ïÿÿ^ðP`AGNfsrq3FGL J1902.9-6745PMN J1903-6749?ïÕ.ƒòéŠ?kè9fOç?V\öCO­?Q ^ÏRž?oÐM'ôÎ2?h³¨¬1?ïÁ¹›ëkÃ?~ބX¤b?7¸#oša?MÑ €7Ù?}§¯ÓXTv?}˜‹H¼?ïl|yF4?Š.˜Ã
:f?xpµs±";?vjìIkÑ?–ÖCêÔq?‡
nš4b?ïß[{.‰?X.dKfæ?FtŒðÑ?8kÁm ƒ?kF°úg?UQþïn4FGL J1903.2+5540¿ÚrKþAu'@4ˆäC‹À7òË/=ÛÀ;oáÔï@gÙØù×?ý+¡nz1?™(Aà ü?µpþÅÃC6@RP.ì|•@öfÏÿ?ïý& Ñì¿×«$˜Æ5¿Ü#Q©ß¿ÜK3o™¿âê+íĔ¿ã…]7»ÄAGNbll3FGL J1903.2+5541TXS 1902+556?ïJT)d]?¦O$üZ­Û?Tfj.û‰?gŒÇnµqÍ?Š ¯åI^?¤ü†«ŒÅr?í*ü҉(8?·úÅ疃Ù? Lù@ìj?°æb*ÄW?­9G,!?©ö"A"Ý?î8X4‡?žç¥Î?—Ý—»sü?•ß›†Zx? ‹²ïÙq?'²œÑ˜*?êÙU``Û?¥'ž Ðêæ?¤Á
ä[èf?'IG ?›w?¾ÔÎ
ÑLø?¤5'ü‰Ï4FGL J1904.1+3627¿ÏÍÊZ¤Ô@*¾°1‹"GÀ9ê7iDÀ<4†6††@ ÔW§†Â'?üdÓSϊí?µÒ
_š~?±õoÙ+ÕÇ?û£¥Üû(@³†;B÷!?î[?î¿ìêg‡?âú°4撿Ûsµ"[ÄÍ¿Ûk:v"¿âQ¼‹6)ˆAGNbll3FGL J1904.5+3627MG2 J190411+3627?ïAøvÖä'?¨¿æùïÉ?O6â•y›ò?`I^3Ê?–Ç:w¡?¨Jm"?ï?ϪR[?œ*ð
'
?MO¹¥Œ?l½›Ê貫?—Œìߨ*?›Ã4Êò{V?í\¼Á—m?£•AæF?i×aÓx"¶?b¬ê€Hä?´K^ä¨Ò'?£f#¬Þƒæ?î{{,'3?Ž,'Vê?iºí€Óõ½?aHG>~?¦¬žf€M‹?7—4FGL J1906.7+5419¿ïõë[¥(@3œ¯¢ðZqÀ;"§z¡‡À<Ò.d—YM@×3ÞLQ?þy™aܔ?Ðý'üft?à'`ç÷K@M;å‰\5@ºÂá¼s
¿äžðP_"ä¿áûR'L¿Ö#º"ˬ;¿áÁI̽¿ïÿÿ)@k*?Ì=Å]l¡AGNbcuTXS 1905+542?é¬*¾€ð?Ät¡6–?¶Ý½%¿
?´uqA<j÷?»Àìêh9t?Àô¯J?éï ºÛÈ3?ÀFž©Ê?³™YÀ¤í?·Ý™e©\'?¼é h|ÑH?°õ[Ý÷¼(?åv lG6¼?°Â³ÏÊø®?ÄŽgMò´?©¥ÕVÝõÓ?Æïç•2[?¤Att‡ˆø?ê݂E»A~?£
~A'?¥d"+Y}Ä?']pO^+ô?¾a£¼y56?Ÿ(ø¨óG4FGL J1907.2+0126¿º+T­–|ÀãªÿójÆÀ9Ûe˜áöÀ;r^‡tÔ@ lû™¾Øm@WhY…­T?Àè%ü¾Ø?ìá~à†?цW2üÂ@ uT•Ùq?ïÆÏ\Êr¿ê0¿»lR¿ÛåÞs=d¿äC¸§Ò¿ê¡É´˜c?¨y?ÜäÇëAGNbcu2MASS J19071198+0127091?Ø|<Ígm?ÃkNŸ!Ÿ?'±2ÉuY?|X¤pÔÛ?ãªýut?Àâb^§k?Ú­l™Ñ"?Ç`Ó1WZ?kawô4Èa?{¦Ñ؇‰?âè;#µ?Ç5	‹gŒ?â²>fyµ?µ'
	À«?¢Vã5[?Œ¹Ðq-»9?ØIØW€iˆ?³þÚ"/;?â´`xˆk?­F@…K´"?‰xQ»ö?xejKå?ÙË~øÜaI?¬üâŲl4FGL J1907.7-1232¿©dtêOÎüÀ"'ãâ"À:|Á>úÓÀ;Ç0ÄÃéÏ@róÜ[50@e*ýÌ=?ÌBÀÄÖ´?°Ïѹñ}Ü?坸ýâïN@4"û§Öž¿ïþ{€©Þ‹?ïø¼©¹L¿èŽÚù¶9ã¿ãlžä²¿å¼ôýîWâ¿äo åRÖAGNbcuNVSS J190748-123221?áÆõ»?‹?ƽaꏽ?Ž'$Ï÷½=?ˆ¶g5ª=?Û}"Ð	Âÿ?ƟÕÅ¢1?蹺'yÉ¿?ÆóRäõ?dgÌ£íj?}v
32=u?ÌÇv‡‰$Á?Æß"4N£?ã§ï%¼•?®Õ8i­¡M?¥j@òD<©?‰ìšŽ©Ï?Öٖ>N>?­íZÔb'?êÔ"û™ ? e€{•M?‡>l=&ñU?sZ,v®›¿?Ã;P*j?Ÿ¡ôåÛ£¥4FGL J1909.5+3511¿ê:MEzð@'µI@»±òÀ;s•ûg¿À<«a«Ã@"•M.²?üzi¾	»k?Ðmµe'!,?²uÄ'aÿ?åP¾ÉÔÊÈ@óß+ôûj¿êwÄ?ì"Ô}›6¿½Mߢú¿°£ýöjœ¿èžHUh?ÐV±Ý³$AGNbcuTXS 1907+350?ïXyT¹Å‹?"n8ÙÓÂm?COوJ€??ïŋ~ôí?"XJéûû?"O.P<?î'íæ»ÁO?°R$j²×—?På5èðå¬?bœêî®$¸?¦I÷äücû?°
¸¾	b?í]©0M›F?˜üŒvG*?v‹hqÇp?i¿N¾<ü?³©½Ç	Z?—ÞçåÅÓ?îu9•™½e?¦–|)»Û?gE㸵L?^!€î³*A?§;'H(žg?¨fI4FGL J1909.7-2140¿ìû%£†5À+BªŸ{À:1"qê('À<O σ`@O'`Âãj@@×¾˜V£?ÄÏr™z?º=‹ÀÔ›?ôîÊ2¾™-@Àö†""ù¿ïÿæ4|ßO?ïÿ=ba(¿ä¼N/7ûð¿äŒ–ç7²¿ÜM Å¿ïÿwåëoAGNbcuTXS 1906-217?îùõFM+Ö?•L±(¦ˆ?w5q8nü?wˆe?šóúҌiF?"ʎþ¤?ïiýë]œò?•×d'aÖ?KRF°<Bk?U'Uo—º?'å°^ʱ?•W·³-ÑÔ?ê]á…\ŸŒ?¨ìžˆîQ?™eW¿'½…?…
lu‡\¬?Ã[Îò¨Š?¦…ê[¿û?íIòCÐ?'Ì'Q¢?ƒ,:
.ml?qÐ¥y"§?³J楱³Ù?'ÑÀþiý4FGL J1910.0-2453?îžèÜU‰}À-Ø$xGÀ:Š'Úb·…À<+¼•G$'@Zx¥-K"@sf³"@?Í¡¢§ŠH?ÐÂ÷+c±@€Xeã‹@©‡‰Ìœü?íÏ~x¿äò]®î?«ªÞU؜¿éRKý."h¿î±†Àyt¿á"Év7AGNbcuPMN J1910-2448?ë,=¯aÉB?»Á2ž?ˆ»Äƀq?‡—×Q"Mí?ÁÃLöÓç?ºbXÚ?îs†¹W¬'?¤²Š$äA?yô`€‡û?ƒÊå?¥¥5Þu&	?¢bö‡Ê-]?éñ+}—ØÑ?¦ˆ>ðv·?®¹}F>Ù?˜@mW•Z?ÀŒòÃ
?¡Ç
0œ?êå7I~? BœUA?–Ëv®û?‡$ûmQC?Á¨´èú§?ÐØðÉû4FGL J1911.2-2006¿Ø­PôAäZÀ*v±=û
RÀ7΋8§À;<18‡0@}ædÌ@×Å>c?ž_ßÛê™^?ŦZݜ'é@$±Ë«d9@´œïd|V¿Ì8Lw§×J¿áÎÕ»ˆ×ª¿æ<tZDïô¿ç{tëdg‰¿êÿ`Ónu¿ïþê šª;AGNfsrq3FGL J1911.2-2006PKS B1908-201?î§ïu±»Í?ž0ñê)O?šœ!_Ôê?˜²¤Û®Ì?eø(h±a?…ešÄÚD¹?î³"&×¼?¶›•¼ŽÚk?•èû"4¹?©2wîÈ_?¤IŠiã?¯[ÀÅár?ìÅþùîˆ?§žbìûR'?¯ô˜
­B?¢´œ
è‰?£¬(VjH?•³iÊ&D&?ì)k½ˆ?§Ó{à¥?{YÁ‰?Aå
T/P?·UЯ&qƒ?¤S:›·s4FGL J1911.4-1908?à(P0NZÀ)Ä£çÑ5À9²×'2tÇÀ<"†4b@ ÁÀÓg?ýªbªCž?¶ã´3gÈ?¢îbÁýL?î,ný@	-ÆJ|¦¿îÝ2K¬§?ïÕdž½Ê¿Þ¶BFÌm+¿ÚNï;â"D¿Ù˜j¥:a¦¿ß'%¡ûAGNbll3FGL J1911.4-1908PMN J1911-1908?ïïŕ¢–À?V*|zü?+²Ê¿Ã
?%1b»+™?\þ"z‡?TŠ9
	?ïÄß]kL<?ƒ€âùákÌ?-ê>Çtïp?@ý.y™?| ÿT;
?ƒ'K'h>?îÜðrFã>?ˆ‹J‡`º?hq©"ÈýD?X

¸? ©ÞBU<.?‡½™v_˜æ?ï§TLè?|7´%ùO?k
äÞ.)?XÿPþÖ6?œôz?{Y'®—ëù4FGL J1911.5+0311?íÔ[Gµ‡rÀ-<ÿdύÀ:¨ÕâDiÀ<"y™I@!–YÉË?þ,\\×q?эM{2ü,?ÜÄÑ¢@
Ö0'?ûóHàn•¿çzá³
Þæ¿ïÿØÝý Ó?ïýÖ$dcW¿Òç*{Ԍµ¿Ùi>›A:¿ïŽÎd|[AGNbcu3FGL J1911.7+03072MASS J19113134+0311093?Ó·É€ï?ÅkûÔÌNì?›Qþ
€Ð?•X¢tŒÉ?åG°áSƒ?ÅVÌҖvs?ɱ$o*Q¢?Â1;>Ø?"ƒPÌÏÍÆ? »båó$?è÷œ]Îí)?ÁÓÂ#1ÅH?áÐþýˆ²)?°ýowáZ?·Šã%û?ž{ìàÒ°?֗ßL%æ?®K90i?Ö	°T†§t?¶#؋‡¬?¨æįüË"?¥dD6ªx?ãl»Š¼ß"?¸ÞÆÀÑÔ4FGL J1912.0+1612?ê–¥F9å@¿2/'À9ê#'¬?À;3³ÍêÚ@Ùà†"@u±ã<zÛ?Òl¸þæ?ÄÕÄÞõ?ñ'þKÊÙ®@<~€¹xÝ?ÒåÇ5樂ë¿ãåî¿â{G¿1X¾¿ärà цƿè‹6"çƒ1¿è	㮐¡£AGNbcu2FGL J1912.0+1609IVS B1909+161?ä¾Géϟ?ĉD–èPò?nî*[î4(?g¤Û€2
´?×À§t"Z?Ä~©JW¶t?èç=( ?Çu¹ããgØ?rÁœ@Ê4?†I¡3å}ê?ÌòV+#yE?Æݱ)xq?æP‰rŸ	?¬¡›±ë·?œ`EŒ@Š?ˆ—"^_?јèÁ¹)½?«fˆ2a?é'{Ÿ\˜À?¯Ïb²jÑ?Zsr?Hw§ð¾×;?ɀñw¦¸Î?¯¾gP‹i4FGL J1912.1-0803¿ï@T.‰À zµ^ñýßÀ8¬™p~îÀ;~^sRÞ@ƹ†sø@"òü~¹?­‰w¸sN?¯wûd9æV?ÿ–xbm@ËN¢$'–?ï.rýMž¿à$åýö:"¿ä—‹')»e¿ã½/
/¿è1ÞõCd¿å',)S¶`AGNbcu3FGL J1912.0-0804PMN J1912-0804?íÊ}À‰È®?¦E"¯5áú?O>3nö?HÒ)^T®_?±máK}¶?¦Pv°÷ª?îö=g³ë?²ß¸®•f¾?A
©´:Á?SDR#Q"?®¼#þÝð[?²Ãfšìõd?íCéLÁºF?š`G=c?"Wj#²]ö?u¯>™Ü¦¬?³UÈU{â?—×h­4F?îÖçă®ô?‰%žýÃ?r¢"¾?_sèAD¥M? Naãƒ@?‡j
ƒ—24FGL J1912.4-1222?âuš
)U±À$n9'ÈÅÀ9PŒAÀ;M¤Ú?|@'ñb~Š@®³Ý¾?¸×4ÀãÓ?ÌÎü|è³Þ@]žvx,@à'i¤‰b?찔[p¿×"¼uf´j¿ã"Àíp†¿çs¢¡¿çG8¤¿ïÿôA…ÜMAGNbcu3FGL J1912.6-1223TXS 1909-124?íÄ÷øJ‹?¯‰žÑ	?›­é¼ÑýÍ?"ªÃTŽ?°®]Ñ	,@?ª•¹¤Vn?ç«Hî…?Ȇl?pÃ
?›PÅS™°k?§k-D¦u?Íè݌KÜ?ÇF‹cjO;?èÐê
.?®(ÖKõœ†?´QÌàÛ÷?¡qJ»w'ƒ?—+…ç]H?¤²W`:Œ?ãQL\tƒ?«Õlùy0t?©‰ûR¯1{?'4ØË×(?Ö,'ÜÁ²?ª9ÃÞ=÷‹4FGL J1912.4+3738?ïÿûìR¬©@(´¡ß¹8›À:š.$ÖyÀ<CLu#˜‹@›C×ñ1@LG䛬?Å´'åLJ†?·Þh«?ûU_]]©)?ÿ|Øm¿Ì?ïîõ üпâcåîy¿éûP£†'f¿ÞáÉÿ={¿ïÿ~›'?ïõ!¬ˆŠAGNfsrqTXS 1910+375?îÎ5KT?®zz"ñB"?‰Õby˜Û?Šã†Éé?¨ʗŒä?¬O:ªá©?èã¥+îh£?Èúƒr|3?¨¯ÆàÖí?²b©Ã>t}?Æi¿^Ž'·?ŊHøG
ƒ?ë°§š$_? ×1£8Ï?šLvŒº"?‰}—?»ç¥p
îb?›½ØÍ[X?êMÌ2Ø®?¨§"`yI?®@¨-Tµ?šh"ã—öÛ?¾qJR0•?¡Ê'žü~4FGL J1912.7-1250?˓vñ4FjÀ$ú#9ÀëîÀ:&êÏS)À;ÑÛ¤$é@ 
¿)öôi@BZƒU?ľªŠ­˜?±5ä¾[?ðãœ*Ù@oL¶çÞ ¿ïæó{??ïzOßK¿ådÂÝ_¿áà³~È¿äxgêŒÑ¿è…2ˆKAGNbcu1RXS J191251.7-124929?éʓŒcˆ?¾–é_Ò³?pP¹¦ƒ—?h4Nˆ'g?ËzTÄ=À?¾c£\¤\}?îRlc'lÉ?³•[Ǩ•?L9D–7uŒ?].>9?ªhT´U?³zƒañ+&?è/ë×}#Ð?¯fû8FØ?—'e°céÓ?'2øž¬}D?ÌN#ëþó"?¬Ô'Œ)|«?ëZY`PF?˜6‰Þ]4V?‰âߦq?uŠ9"£—Ò?ÀøoĆ?˜N@â,pÑ4FGL J1913.0-8009?ïŸX1ªÀ;žêúµ=dÀ8ãÜEԉÀ;·%;ù«R@yiÓ®=k@±ƒÞFqÔ?«Îªžœ8?ÂWzzÅn	@§Òª\_@:Ë-?€{¶@ˆ¿ßÓ þ½¶¿åìÉ⌧™¿æáìï'{¿ê{÷"J¿ïÿrÁ¾{ÑAGNfsrq3FGL J1912.9-8008PKS 1903-80?ïÆ''ÿô"?o#ÙÄÁRŒ?c;Âî—Ù?]Ò;5ó?sN¶Žië?fÍaSPo?ïÂ\Yþ^°?|·t­Mÿ??7GK{>N?I)…íc
?}]aô³?{¶(
ò)Y?îü\Dý?Ž!9æì?€\/‹rø?}¸QÀèê?˜QE
1¦õ?‡.PÏøé?ïȟ™ï‹~?dtËP¯Ó?L dùªC7??Q\ò`(.?x&iù?c2Uú
F°4FGL J1913.2+0512¿æ™5‰W_ÁÀÊ›š$ÚÀ98
¢pÀ:ÕÈ­ç.@ÀŒL©ý@úo?Rü&?Êj»ìÕ¬?Ë­G`ç¡d@¥s!_Ì@KÿßÝ6?ïJ|€Y+À¿áU)' ¿éøn¦¦ÈV¿æ¼o»¿êě¥ãSø¿ïÿI)>¾AGNbcuTXS 1910+052?¾½pÀ¨ ?°¦«ùÓÃ?°ð˜•Ô?¥øÄã'°"?ê &^äB?µ¹äùN?ÃW£äGèÇ?ºÆΣ
#°?¤8ay9­?¤ùš¹ÅXi?éæï]Â4?¼R¡B	%?ÌÏÀÍ#ú'?§€|‡÷õ?¾?Â5_|Ä?Q#`Ì~?å†Ç?ª~¯º1?º:YÄ¿&Ñ?›ë¥z̨"?³	ù`ðn?"16½r?êWu›J
b?£–óäÈ+$4FGL J1913.4-3629?Ôðýsˆ¸ÌÀ3ÚªŸ{ZêÀ9³æ鮄ãÀ;'ŸJ³'@ë€nÐBM@$FE^¯?»ßð¯š?ÅÀüI'I@ˆ=ÿ?à@4¥/úĂ?Ѫƒ ÜD¿ä"²ªØ¿Ødñ†Ày¿ä'Ù‹÷ð¿èÈòýãñ¿êy
By!TAGNbcu3FGL J1913.5-3631PMN J1913-3630?î½¼'ÈSt?ž Mß?Œ?–xw/æG£?""Cm Dž?'ÏöwIç?˜3îÆå?ï £•l?œ¬§€î?f¡"†í^?x¶†ãÒ^?™k|'&Ä?™°¸ïNž?ìBCº­	8?¤%u?"ÉLéè͋?ŠZNµI¹?¸»Žð'Ñ?¡L`ô¯?éøqF.¸?¨íU`Û ?Ž$~
?~âÛw+4e?Éì
(žM@?¨m¹2¡…l4FGL J1913.9+4439?í;´î×,@-ó*k
•À:I¤¿g‰|À<t'Ç=@Ó@£%2g±?ÿJ£ý ª/?ºK_ú¼t?©æª!.×b?ðs
=Ö$@*fÅû?ïö Kºi¿éï=n¿ÒeÎÜŸC¿Ù÷½j.G¿ãV½¢…¿çT‰Y°u~AGNbll3FGL J1913.9+44412MASS J19140184+4438323?ìÒÒ³òP‰?Ê«°×dÝ?W¨6ô3?R=Òá"Ug?¹
Ʉœ¯ª?ʵÖ	ã?îï×ôÚäú?£"†Ì›GÚ?\'ÿæE&?mÎüŸtÀ? è³¦8?£¬ÿA5?íÀ:
s‡c?"b·¿bz?|©€æO'?kÅí˜IuL?°3—…þËÖ?'–f?îK<ÏÇÁ*?†–õzÆÉÕ?…÷'$=Õ ?k†ÜvªVÂ?¥ÎRztx'?"(q<¸N 4FGL J1915.3+1149¿âïáÙ?ö}*"=mÀ8vW0h}˜À:º|h0@љÅäPL@k9ýQÏÖ?Ã`qšL
?ÖFíD'o@¸0]•Ý@™Õ­œ¿ÔµŸ^ª…O?éO/]e¶¾¿æ	!ay—œ¿èy‰Ž‰›¿ïþ›{ñèæ¿ã¥ÁX¨8AGNbcuTXS 1913+115?ƒIaâÁ?"©*q•ö3?×.'tÚß?Ê¢36
?ä€n ?ʹ•¶D¯??Üdné+?Œ*™•êZ7?ÕA…ç릁?ÅR÷h¤¼N?äçË{¬q?Å*é0€o?ª—V7!¦¨?'h´ýs¤±?Õ_"´k·?¸}4áˆ?ã¦ÈBX»?·³9Ð<%?vLÎçòñí?bïZvÞËP?̝ºá¬¦ï?²@ý‡CÖ?è«÷©Äð`?²yiŠÍ‰ƒ4FGL J1916.7-1516¿ï÷ØÒû¡2À(Èõ\)À9ÌѝìåqÀ;ÄSõJšX@#>¥ØW@oúcÞÍ?Ãû×ý,'?Ðô!ºåĕ@ð@|ÇÑ»@D]ÓG?ï¶A……¿áøŽâ[X¿éƒ†="	¿èTÒõ۹пë¨"HK¿ïû÷"IôAGNbcuPMN J1916-1519?ï€Íý֜G?­ÓžÅ™š?zhWu‹?"ô¤È‡U›?'ËL^ž&'?£¼Aç"µè?îèÑtÈ?¦ˆÍ±\44?pVÒòۊr?V¾ö+ki?žéq·$g?¤ƒßèò%?ëZÜw6W?¦|ùÙ²‰?¤^ƒO²?'"mó?½z¥p?¡d^/™C?ìœÌøý!b?œs®QZ?'#J¼cþ?z•R+W<?¶ÐÑågÛð?š£ ñ҈¯4FGL J1917.7-6442¿"•/®l°À;•»¾‡À;	ÏDvQ–À<ªJaÎ@÷\"ë'`@œ2?Ñãâ» ¨?ÕP–ñH­@=p£×
=@'ŽÇ®Û¿ïÿÇ*Ì\e?ïþΈ°=¿á%Óύd¿çòùℚ¿ßë,~Ž%r¿ï¿ü¥¬¨AGNbcuPMN J1917-6435?ïúrI?"1oúÁ2?p^ŠE•Ö ?ižÈC˜?š	,ºl?')&O| O?î—$[Ž¸Ø?£Á¥AÒ½?p›ûXÅ?zòY+Úb?¤z:ÜÙ?¡õ@æþÍ?ì!O•x? [ӞÎò?¢˜e"ú*ˆ?Ü"
k?µ«ºÀÚ6ù?—îõ‹;fÐ?î<™³79?ŒðPÁQô¹?".ùò#ØË?r©Œ/íE?§*¦P†1?ŒMiÐé¾@4FGL J1917.7-1921?ê.Ü2µ"ÑÀ,¥(IË%-À7õ"i†¬WÀ;jUõÕÛ@âÈހ©^?þšÈ:£j?šlûÅ¢zØ?˜\ÄÙ?üp'|F¢@:ŒÁnö?à­ÆÂqª¿Ò‰½#ã4¿à_Ðéſ۞üd¿ó ¿á5Мe&¿×èÔjOÿóAGNbll3FGL J1917.7-19211H 1914-194?ïÈA‡ceÛ?q¶uOè¯?7IüªÄ{?0ë%*é8?zjœƒ ÉA?q8²Óä'
?ï¯q:ðgU?‡žã&ñ—»?D­¾¢­¿?Uöë%ÖÈ°?'ØÕYÄ A?†bo&ØÒ?í¯Šã¡7?žæ©ª©¤?wï6B!?s×ï'!r?±¤µ~Õ?a§e6¹Ž?ï'—uˆ?ƒuô"9ø?qJÔgyÏ|?bÌ14p·?–ºh÷pˆw?€ºX§'p4FGL J1917.7-6930?è ²ÕªÁàÀ;' hUSïÀ:NãF¶žÀ<p(ßó@Òë1¼»ˆ@SX"?½qõ:Õ?'Ç]~4Ê?Ô$ þè¨Ë@
0#	ÅP­?¡UMºHä¿ÛIÞ}¿äzï,D¿æ8}¿H€¿ãÈM Å¿Ñ×DÔñ4AGNbcuPMN J1916-6928?ï¸v…®äv?uqØôoG€?H=Y…n`Ú?=AmŽa?€^ˆûïü…?t˜ÑS(d?ïÏïŸQ?©?x–<ç_8¬?ØV¦þ?2·ô¹1¶+?wˆÎ[&ÐÓ?wå"…Í~†?ï9ÀW†K?€Ëó&§Èk?lIE\D?\¶­-íP?˜ø>Ìc¦å?~.Æó|s?ïØ¡0¨H?ZJð°¹*3?;ðÌÇÔ&D?(̞7ë?r5"›.™%?Y@ÍcãÖ4FGL J1918.1+3752?艊^N{@&à=ݱ ŸÀ:Â7n+VÆÀ<vÒõÛ¹Ð@ |ú<ü¶?þÓCßRáN?Åb}äzC?¿H‡h:&?ùf'•ù@sBdÔjü?ïùfˆË?ï³!å#¿Ð_¾+Ÿ@¿Ý0¥dSÉ¿äD-÷Š¹¿ÝfN=¥§ðAGNbcu3FGL J1918.0+37501RXS J191810.2+375315?ïIU£—
?')±A?\C÷û‰Ø?uiFÊ¥Z?•+ԁ?'K_«˜?îm•¡âK?²ԃ{é	?X@‹þ­y?lë¾2g?¨d¡‰–Åà?±Æ¸Ã¸ˆ ?î
Ö
!3?–òc' ?qú&>ºL?cÓ«ùQo?¬ãZfŠÕ?•ÁÛ¼­?îiï²:®?ŒÀ7¥|£?†øÖ/@Õ?wÐçBÄf?£¢ÿ&Ì4í?ˆ°ã24FGL J1918.2-4111?Ê£üóAgÀ6=cEI¶,À8^&åGÀ;wF'‹ˆ_@3,éŠ?üíy¾Ô?¢ð"½DC§?»œÝø©Ê@ãÔHµ{@ó8–õOx?±
9>æ¿Ø6êx´G¿Ú
Jk^ì¿ÙÖØ9¦ë¿äw^o¿ç;C£AGNbll3FGL J1918.2-4110PMN J1918-4111?ï¬ÆEˆ?wûOa¹±ÿ?UãC¿¢/?V±Íï9Æ?'<eüÅéÖ?uŒ›Ï Ü?îþ4õHÅ?ŸÆô¶4³Ÿ?tž˜ëY
?'¸lÔÞÖ)?›"&€¡?œ˜µ°Éܹ?î8§t‹?œ"è!|Èû?"zfOJ¢†?ÙĖ^¬
?¢B'aÕÿ?"±½D5–?ëêøør? ½{®øŽ?'kíA1E?v3¶ÂàMz?¼üÚÁˆP? ¸Dëcë4FGL J1919.2+0618¿ä)ÞTC#À
!ÇÃx5À9wEšMôÀ:ö@&t@õøADÃÔ@ïOP ?Ù*æÞpä?ߋ:[E ô@	áZùJÚ@ÉIýúí¿Øí‡Â׀…¿àâeàÚuØ¿ê"¦žô:¿ïÿÚv»œ?ïøÍaO—¿Ï€™XG#AGNbcuLQAC 289+006?ËYb­;ùØ?ÀH÷‰e«û?§Ø&îšã?§ÙjzÜå×?ç¬$åÐçÜ?ÁçC'?ú?ÖݦÒ—å?͉ÆÔÊ«?""FW8M¹?§™ô}PK÷?ãðd=ñŸ?̳d+#?Ï΁sy÷?ªÉ‹¥S?Åð{á.p;?­á ü¼Vª?â@ªóÅs?±ôÉ)™á?á&ðz:&?Èê•ÿ$9?cí¡éý?lRÙry?݊þý°p?Èèù`êÚ4FGL J1921.3-1231?ï«ãÎq»À(|Ä&5ïÀ9þ‹‹¹ÝÀ;ÙQAK$@ìÀÜ©Ž¯@$'ÇÅ&?°€m"Ã#?°ö AÏ@0
ø'@ªÅÎÖ½?çÏó"
3`¿Ðÿˆá»q[¿âA:û¿Þžœ)¥ì¿á¿ï~Óo©¿äҌ)nŽSAGNbll3FGL J1921.2-1232TXS 1918-126?ïB¼ë˧Ô?‡Sx'Ö!à?d[ÁŸÝ?YÍ2ÅN?•&W	¯?…àE0ǪÝ?îØSHVŒ?¡ˆT€6W?kòÖmÀ§˜?wl£¢Ïßd? »ž»5? &¸|Iø?ëm­c7ó?¥ãøÆÏ-Î?'w×ZÛ8?*j2~?Àg¸«ÄÎ?£Ñ˜"ʛ$?ë•Å|8D?›{l"‹xÇ?£Dš}¤ÿœ?‡#:È5Ð?¹¯†ßk[Ó?•ÓµÝqÑ4FGL J1921.7+5817?¦,XnC9@3	‡¤¤—À;Ãú%Ëk¤À<õçoæAé@!×Û[/ür?ú}$ƒmj?ÐÃqnØ$ð?¼Óæ``º?ñ§Sçáv@öh@†-?ïÿÍ?¹Ss¿ïÿ'ÌÎzL?ïÿ°ï÷t@¿æ#Ã>-¸¿¹øk µW:¿áG»ëÓùAGNbcuWISEA J192158.68+581708.5?î>
ì)j_?°âÉ&}¬?PH.ö†	?R¢
l"Áê?«œÜ»ñ¥î?°¿O}ó[T?í$ÇÙ2Ï?¼óŒKz˜T?u]ü='5?†¶÷Icw?µƒár˜dž?¼~lÛ#Aî?ìiF²k5Ñ?žö¨Žöî?|&[&†?rŽ^Zo?ºëøóïÚ?žBYþ«¬??ìüϸ1Ñ?¥üjľÚ?aBa"™t?cxîCh?·•&v©I?¤â<\4FGL J1921.8-1607¿îšŸÅúíêÀ+¾¯«SÖAÀ9NjXŠÜÀ;¹ðál—@ )`^dL?û;=Žc?²c/¾ù>_?·m?Énžn@Ѭ€&+
@
ïß´tç?6ä•¿£Ó=@§¿ØÕD€ª³¿Ð*b{ö¿áa'Ú¿×IÅEïÎZAGNbll3FGL J1921.9-1607PMN J1921-1607?ïç˙ŽŸ+?ZaZ14ð,?1àm¬óbY?'z'«Rà»?eøX»Âgs?Y3‰"vç=?ï¯a¤¿l?‰ÿ"·eI?;x€Ý%ر?USä'œz?ƒKÒôfõÇ?ˆ}<«âÀ­?îÁÿÉT?Œü4vd?qk? bë?hT–
܄°?¡²›Š*M?‰ÈÒTºŽ?ìðIþD«?œa¨f?t«…0ìÇ?aj'Kü?·0Ý]Ëà?›÷ kþà4FGL J1922.2+2314?ì2~ZŠ @!0¾
í)À9Ò°@¥¾À;¶_ !¸@ ˆaV݁@x˜:	?Â^´Á=L'?½Zž\! ?ýEª~Ä+>@âw¯äà¿ï²xË'u?ïüá½tÀ¿á8&êþ¿ÛT÷=¹žó¿æUF˜¶›¿àjëø?AGNbcu3FGL J1922.2+2313MG2 J192213+2317?êoŸu?·ÌT^Ž?{ÕG¦ôP?xé$¹FÊè?Çñ…¼J?·wÎ"މ?æ'G‹û_?ŹÂh{€?†?؏#?•–´rQ‡Ê?ÒKfë)?Åq2šÉ\?æL^¾"ñ°?¯"¶Þ¡ü˜?žFimOù?‡·—é^gË?тÛó"G¢?¬ÅiÕº
x?è\·ƒ$?¡ýùÝÎÂÐ?¥¦ÓÓ`f?šËâ
?ÉJ8>zÇá?¡Z"»•iÕ4FGL J1922.5-7453?ìoD'ª®"À<#ædM‡À:Õçþ{À<fH;Øô"@ Xr…®€?ýA"d~.Ú?½î^Aÿª?°!a#±`
?ógû&|k‹@	™Ñ;Ü?æ|
A±ü¿ã¶Ã«»Û
¿â2§Ý!ž¿ÐJoD³8¿ãâ"i·S¿¿Õa8¿!œAGNbcu3FGL J1923.2-74521RXS J192244.1-74541?ï衵ü÷?}IÈoóÊ?/ø Ì'ý–?6øåM瘯?eîÔ=@ˆæ?{Äó"â(?ï²W¡~+?ƒÝs%LÓ?2yÍ
Ç«±?Fã´]Üö!?'ÖIP27å?'}QËý_º?ï-mšç(?}ô¬ÒÅÀ?`ˀó?GÙ	*×('?˜DHáZ&?|xxéÊê?ï:Ôü6X¶?xóúñ.Ð?e'•R‡3z?RŽ'øÛú»?•ó
Îä?x2ö¹	4FGL J1923.4-2503?çÉ½ßÛÀ1ÄþG™ÅÀ;w/âEÛÀ<£|§‹@"RßÛGcí?Ø©Ý3¢D?ô[D)$¼?ïÖų,é@X> N¿@`̇­ˆå¿æ¿ŽU˜¸É?ï"Fj^¿á/ÿ¢/?ɅsFô†$?Ætð'^"‹¿é0…;=ÄAGNbcu1RXS J192325.9-250228?î¼¥ë}H?£Mº;
jB?Ž?‡Ah?˜V–¾Èï?™K™B—O?™iXËh†T?îÀי`¾?¶kø€è­?hš}–Só‰?Œoð©r>?¢hސŽÞø?µá¿´Mr,?ì²Æ.ê/?œ_¡šLÎí?"Nàù÷?‡nÃH3œ?µ–*q·?™-]ÉA~?î[ºRxÊF?£¿"¯™þ?PAß8?;eõ{£Í?ª4²·éM¼?£Â«Lxl4FGL J1923.5-2104¿¹8PtJ/À0>îؐOnÀ8¡Ïi_?+À;¨''ûÈc@øÄI¦@	<Ú{áù?¥òÀ§Oµ?ÁÒw[¬#4@ù&âÂØW@0—d54?œ!¿Ýø¢¹ì¿ã×Tæb¿ãÓ?ãDÞV¿êüí@àšà¿ê«hÎör¹AGNfsrq3FGL J1923.5-2104TXS 1920-211?ïK²»pŒ?†'b€S?sxœyk
B?r.Eи?'«–j7+È?'_9ow?ïՉ ø—?€!üwL)?,ftvj¿?A<Ë#³¿¬?tWûˆÅf?Éz¯…¤ª?í
úâ€	+?¢®R²rr?ªÌT®K?œ[¸°8?¤Sý)øÜï?"ÄZwiå?ïï-
vôw?QÿUò6$‡?ï†l×ÃN?ì‰ÇËû?_¦ò«I"ý?Qf|ëù24FGL J1924.2-1549¿ïï"îJÀ,†)Ø@žVÀ:õ™ÊARÀ<EÏ¢j"´@ È¿èbÕb@`b
·'?țëƒq9(?—;ƒ8Ú.?Ó ™?׆@k¨÷/¡Ù?ïµ;K/©;¿ì'Ë $c?ÞQmü÷¿ê7‰Úõ¿œÚ»ç'
¿àõ¶€Z-sAGNbcuTXS 1921-159?í3LÚ}xd?®†ÛëL³?\ùwäž?X¨a¿{LÕ?µõ}GÚ]B?®Må[</'?î2˜µÐ?¸¼{ÚßjJ?`£4~½Œt?rý$²&?«ÌLWÊ7?¸…}Kú†?ìZSQË)x?Ÿ8î[?}WÏмij?m6±d¸[?»Wètšíª?žeE!Ûô?ëNl­g?©¸FO8M—?Z‹-*'?Y³ÊêUâ_?'9µ	/?©ºÜ~áË_4FGL J1924.3-5458¿ïáԤÀ:"œT]À;OÖNUÎÀ<Ãü7ôc@ I£ÿyw?äԌê^®?Ú|"zÔ1›?‡ça@9ÞýPù@'²¶v??àbñNŒU¿×AV¨¿ê\vXKñp?ևáá1à¿èâ¬K¿ïþ Eð¥AGNbcuPMN J1924-5457?ï4‰š<5?"—¢çTI5?xæOþ€§?v´å¸
ƒ¬?"5Fd|Ù?'wF#rÎv?í號S?¹Þý¯>¶
?•q™«'¥9?¬öߧLØ?²TÈ"ü?²©
ú¼
æ?ì©2¯¿…@?›Â"ïaç?—Æð"}?ˆ=î(U~§?´Ä®]#'ã?—x0ÄIáÅ?è5ˆ².%?¿´½ùAé?'ËÞ¨,½?£
E¸ #Á?Ìðd¢AÖ?Àƒmè14FGL J1924.8-2914¿ïâ]íúxÀ3›ûz_A¯À8ªX-¾À;×/¸ToÄ@ú';‡@ò\f2d?¡¯Šœ¦"T? ¤!²Ø/?ø.8øo@‰ê¾ÒŽ¿À–—Ü€¿â‹…Û¿æþA¹Þ³¿ã8î~Mbß¿åÙv0¿ê$-ÁÚ*ƒAGNfsrq3FGL J1924.8-2914PKS B1921-293?ïÝÚ_Ttœ?f ¥'ü"ý?32*eX¦ø?)(¾Ý¥J?o¿[^àNç?eî'ÆÓ­Þ?ï֏ëxÐÀ?yÌ0ügº?0
s-j?LÉi"%?s¶Ùlgw?xÂBä<˜?ï0"{?‰wZyk‹?pŐ1ó%y?lYÁeý9Ý?›ˆ›o3Òé?‡™"šâK?ïñŽçD1÷?MvGHWr?/t»J¿é?$ñ%Ë_?¡?XóÀ2»à?JM'Xv¢4FGL J1925.0+2815?à-OJ"ÍI@AS½vdÀ9œIlÊ.À;þ)ÊÔ¥@ W)HΦ?ÿW¹Ëh?´øá.-»?¤ý"ãél?òÛHZ⤥@C ,pKm?ïÿ"å­nc¿Î‡ rÑ®´¿äOÉkï<¿ÔrÔ§7¿Üø°WK@¿âÁ6á¾vsAGNbcu3FGL J1924.9+2817NVSS J192502+281542?émÈ%°?¶±ïO"b?{¤'Ÿû?mdée1¡­?ʽ+Û¢pk?¶p¶¶¦œ?æ¥þ{":?Ź†ûìd?uµ kyŠ?"¢%ÄI?Ó¢},‡)¥?ij_"vó3?èšËbÔG}?§kñ"–¢?–
ûäË?}ªG‡s?ÊÓpµ2^r?¥¥ôÚ·và?ëKa֊"N?˜fXý¡Ó?ž "·ö?ƒ¯y~àÞ?¾=iCÍ¿"?–vÓgõ|4FGL J1925.1-3358¿¹™›ïužÀ5H¹ý½/¡À:qè«O¥À<‡çÀn@Ôíè¦G'@ԏ¿%D]?Õmfr{?ÒãízÂ=þ@lû%¥«÷@•POù'~¿ÆIà‰B3¿ém2}«§c¿àê^u׿ïü?OQ¿Ï‹Å›€$¿ï©$Q ˆAGNfsrqPKS 1921-341?í±J'¿a?°K
°«‡ý?e;«^‰öã?a™²ÊÏõÉ?±ËÎUI?°‡ç ³¦?ïÙv°?úp¸éFj?e÷ ÀE:?vI†ؒ—?œÏµè'?›šÂ½?êќ.™<ë?§áK'.6ˆ?¡w÷ë)ƒ?Ú›Tޖ?À['JÐÉq?£ºFϱÎ?î´??¼?‹³'ºzxƒ?G>';=?Ab 2	"?£wùÉwE?‹kE¸UM4FGL J1925.1-1019¿åL5³@3ÍÀ(@^_0çÿÀ9"¸:n×À;†¸›½`H@Ì®EM<@Ò<B¦m½?Á†Ë¡(¯!?½lvìÚ^@`GMœk@¯Ôà—"ì¿Ùû/€÷e?ílkûѝ¿Úö` Éd¿ã,'Ž2]J¿æ>o;÷ýÓ¿í0¯_Ô{îAGNbll1FGL J1925.1-1018PMN J1925-1018?åpñ2ߔ]?Ã΃âÇ)?œ'ΗÈ?œ×	·Èï®?ÓU
MWfê?Ã.¬s×!1?ëWON¨©á?»Ë3ðݤ4?©7yá¤8?­@2"^\"?¸©È™è"ñ?´¹èIC?ÝÉα°§'?´ÒÛepÅ?­ehò('?'8&QM"?މ"0
V?³±Üe´¯€?މOˆ©_û?©e¬.Lø?»Q
{g~?Là;‡H7?Ú´Ü3÷Æ&?¨ÄÁ~Ì
4FGL J1925.7+1227¿æs·8L2ð¿ü†«pÀ9á²7QÀ:È[;ù@¸žÅÓ^a@§;ãÛÝ?¾TÂ(Y?ǸMú3ã1@ïƒæ©í¥@ë9Û׿ÁÙ}µ7"Ò¿á¡Î¡¹"Ì¿ãȑûž¿åªÆÇ©¿ê|=2v¿æÍÉ¡õÔAGNbcu3FGL J1925.7+1228TXS 1923+123?çnþq?Á
*ëó¹‹? •±¼¤\?—Ž`‡
½Ü?ÏÀ×ÂJ˜í?À:¯¡˜™I?ãÚEiºG§?ÌÓþÀx^N?eïªãWâ®?~ï?ÜW?Ø•ÖÄÀí?̟iE®hI?ãcÚÎöç?´1ñ€y?°"ےøà?šRñ:¾a?Õ«-sÃ?²>µâ´)?ân¼ð?¶ËõK´žã?z9WrE‡?jèEØ
?Ûjµ ÂÎ?¶ÃÞªL_™4FGL J1925.8-2220¿ìlS€ÁÃÀ1?´åOz'À;GoçïhÀ<ˆÇ:¼"p@"!ëu(?û¦Ô€u?ÎMoÊhC‹?³¹? Só?笇²çHy@'Eã-¿ïö^½|?ï±Oޏ—ã¿à]LÁú‹Í¿Âï,ÉÍ¿â¢y|¿ªYÆ<\I$AGNbllTXS 1922-224?ïIJ ñæ?sµú·x²ò?+åk¯¾¯h?"9È3ÅY?|àûR	?swý+.‰F?ï=¥ÒÑÛN?œêJÍnN?R‰ÄzÍî#?v)e‰èSÙ?—"©^·4?™ÄbÁü$Ö?î-‰Îǂ™?	x㳏ì?mš
ÍäÔL?Y\Ä÷ÉgÉ?«MÂf©‰#?ŽþN?ìYzŽ'Öü? p@æt?tžãåŽý?j£XÈÇC?»êJMªï)? ,¤&–Y™4FGL J1926.1+2059?Þ^ìD®±@v]¤öÄîÀ9†V›HÀ:÷¶‡æê@Ð"—¯Š@ž9ÛT?ǟ¬ƒ+C%?½Ùß‹?øB;ëh™?÷ž§ªÿH?î+h~nšè¿äIî*ëf¿æWð}ðÇ¿åâK^Τ¿ï°Ö+ñ'¿ïý,ÆAGNbllOV 239.7?Ê<¹E áˆ?¹"ÙòîM?žå'tÔl7?­L¸|†ãÀ?èy¨s$<?¼ã÷ÕlBþ?Ã3Q‡Ùs?Áö–´ãž?µúƒùK}?¶e'Ê@‹Ä?è{¢¬t•ô?Å#;!ø4Y?Ïø°¢Ìí?«=p\úNþ?·tË`¶¡¿?—­t±ŒÁ#?å:kg¸Œ?¬3†×#€›?±ÅÏ#s·?"í'^àX?½`Âmá5U?¡!`VU?ê-ÍÕbv?¥<S€Áú4FGL J1926.8+6154?âý˜¸"Qš@3¾š^»w:À9ñ\Ï
ðÀ;Îm=ðüW@Ã@7ü?üŒ•¿ðEx?¬« Ðg?µÜÃdïû@|XƒNÔy@>C">™C¿ã`䡪µ ¿¿öÔ]9ìá¿ÜðÄ£ÉH¿Ør/ÈD§Ð¿Ûwp#ÿc£¿ãZã±àbAGNbll3FGL J1926.8+615487GB 192614.4+614823?ï쏭|?cƪ0¤?=9Ž†'# ?8·¼ N€µ?`Vȟ€_
?a¥ú/¨Ø?ï—é0t†þ?‡§Hø¹Vb?S"×ÖÄá?b~è8«»?‡•è¤œ?†	»FhÝÚ?ïñŽî¯ó?½³R?p–¹÷L?cwD"h§ˆ?˜<LóɃ®?~›´*ŸÓ ?îäã\‰!B?€²ÇíՇ?ij³Éæå?TF(‡ß? úςò?~™ô¿Ȍ4FGL J1927.5+6117?ª‹:!&P@3qí9SÞ¤À9d²<'ÎÀ;îQ°Ì¼@s7ævA%@ÞÄK?¬l«`&Âs?³"ÁO"ç@+
=²é@
¸`Ú
x?ï÷náàb¿Û&¢+8'ï¿á½< —¥#¿ã;©p¨¿ä{`H•¿â¢^d9eAGNbll3FGL J1927.7+6118S4 1926+61?ï³1z؟Ù?x+w
Vþ?UY¯×o)Ù?PšKˆH0?€ˆkNê$o?v4%Sš§?ïnT¬Ë?Ž™ËÇÒº?_K[{ºY?lŸìSº*?Iß¹âß?‹¥UÜx?îæFbЇ?†AO»1=?xe­Nž@?mÓ¨™Y?È|ÒG"?''=Ù•?íáˆàÔ©
?‡öBYź?ŒVn¬·«4?q
WCdžè?ªÑÖG‡"h?…:CݘK4FGL J1929.4+6146?â~rµV`@3gag#$ÈÀ:t+'~B%À<'z@¬Þoâf@$&5îþ?ώÜð±X?ÃÁ• ¹?úNêHޖ@}}¸'ƒ%?ë™.9Ï/¿ÝÖUa±Jæ¿èÚò)}¨¿Út°`Ûb¿íޥœÈ"¿ïÿ±@LAGNbllTXS 1928+616?äą*È?ÀWÝJ-
?¸?zzVM?¯OQÕ¼Kú?Ðg
wZI?½Ô?eo?ë;uÚܵ3?·?‹GNÆ?¥þ_3eA&?«%õì㛞?»%!gµÚ?°¤æ¯¡Úv?è'#dk‰?«Ç6w?©ðŠfîÝ?"À)Œ™BÊ?ÈçOԘF›?§Ñd_`ÆJ?âØÓÞ³O?§À'Î2·Û?¶Òé?¡«‡:¾K?ԙÒ~{"?¨p¡¬oa
4FGL J1930.3+0911¿™»£žoÀSÛ]‰HÀ9)êFZWdÀ;ñ`®—@qÇO_c¾@8þžÖð<?ʋ ÆÒ?ÕC!ór@Êôj ‡Ê@8ú0³&3¿ëœA^ïúy?îâþgy‹Ý¿ëyIbI¡4¿èÑ[§Æƒ¿ïû•!ººÑ¿Ö‹N<Îè[AGNbcuNVSS J193016+091037?ààO³òi?Ŷæ"A'o?¾'ﯰX'?¹²r¹ï~E?Ø-Ãt¬?Ŏ —œ?ÊdÅøP¯?Èdº¦{5?Íö'´];?È`"Kû_†?áé-Ôèüë?͸Gþ¼'b?Ì¿«ž­##?­.܏º|•?Ä7mÀþÞ·?¤5@"ùÿE?ãÂ9¨ÿ‰?°y^ûn²A?СCÍÆFõ?ªßÍç?Õ¹ÓÈ>©Í?²ÀõW\¯{?Ù¤èiû??°òÞoÀ54FGL J1931.1+0937¿Þ¸©‡Ö×À0É°·À8=éˆÅ6À;2'î"­y@ ]ꟸ?ûfÙRí
?ª­NWPôº?¸OÂ5<g@Fß?–@ò…-H?è#qߖS¿çè| åhO¿×ùÎøö÷C¿Õ¿r¼`¿Ún?¿ÜaˆE´?7AGNbll3FGL J1931.1+0937RX J1931.1+0937?ïBZ†äV?ŽHK'0$_?I…×)RP?G$J~‰?–ñLˆj*§?¢\Ô&â9?ëZ'c«"*?ÀTÞOÅD?Kù‡‰²'?e
_ùL'?Ây¼éȬ¥?ÀL	nÊ?ëvD ¢?¦ÌôD­Á˜?÷ü‹—)?‰ÞÁ'TW?À"\
–Ø?¥¬Jì¹4?ëY)ØsU›?£Êöô]¤?q>4þ¤·Ù?`0–"oZu?Âfö=ƒÔ?£—‰GUÆ4FGL J1931.3-1556¿åƒEßÀ/¾PÅë1<À;u–²^Œ}À<Ú.Íû¡@ "´+?û=\ÿµW?Ù6¬Ï×CH?ëpý
':@¹ÿ]BÑ6?ÿ¨C0¬E¿í"½«;X¿êº¬(©l?ïó€`°?¦°×½…uå¿íxa"·¿Õìò\(téAGNbcuPMN J1931-1558?é¼¹8ÆP*?À¼SbÌò¤?«7€ä' æ?£:q¢ò"y?Â?:ãÂW?¾5<d#½Ü?鄣©O?Ɗڊûàg?¶¢Ÿœ.ds?À٩ۀ_w?½8Gf‰!?»ð矐Ž[?çBupî¹é?°*
kc^?¹5ñ™Ô?¡K;LéÙ?Æ[1¹ø–ó?¨`ÕdÞd"?äóø³îg?¹«ô&?¸ªGBò—Ø?±ŠÙ£V®É?ÏÞx{¶úv?¶ˆ¨ÍÛ4FGL J1933.2-4539?á¡ÞÊPE¾À:	¥e¶šÀ9Ð]ÿ—¸À<3Ð$ër@'.ϏÐ@Ïf"‹?·èÞü$SF?©¦>(ëÃ?íÀ‰þ#r@
ìª``ö¿Í…ÁµíbD¿å¬°Í'Åj¿ç³:¿ïn¸¿åíLŸ¿ì¬•à–¿ïúï,DAGNfsrq3FGL J1932.6-4537PKS 1929-457?ïád+…Î?gÑ<X;¦?M³~ò?TÀü'×?gZ'ZtÈ?bv§7Éò—?ïÅ+V0˜7?Õ@¿ÔG?0€Tï1Ý?D÷¥ÕÜÊ?|bO˜ÀÒ¦?~WG•êÍÀ?ïW{ý|"o?uï§3—@l?j`	»Dï?Vl ¾\\…?'Äï8	‰?s-OÓËR?ïÅYwYW¾?c¡¹ù‰?ZL|àiõÎ?E×Ñr£ð?vÀ%9£Ù?`ýþ5¤–Æ4FGL J1933.3+0726?íxî ï†ÀM;€ßŽpÀ9!UŠv(À;½=1¹¶p@ ß6<ýâD?ü`¬}¡ìN?±4è%ü¿?­M	âÆ£?þ(³}pn@ì{"`'?ïÿÄ;-Óx¿èkþ‹‹¹Ý¿Ú®(ýân¿ÔpŸÌä¿Þ¾"¯<C¿Ùyª	bAGNbll3FGL J1933.4+07271RXS J193320.3+072616?ì÷­ñ+Ï^?³MíïèØo?Rh01[?I¹üDø?·úX1ÄH?³;Ó/Þ§$?æÔWâÛ΋?Æ/2Lm2?]±ßä£dð?oÇ©§ŸÍ3?Ò9žZc¿"?Æ!*½xÎ.?ë&";Ð ?¥"7îŠ?…0"ÚwçM?t}%曜?°æ	A?¤›Úµ¢­¾?êwáÆlr? °Õzë;?'ÉÒ…x.?zkñç1áE?ÃÊR55Ÿ1? ,B&®ÿ4FGL J1933.9-1025¿ïüÃ~*¹xÀ,;}æOUÀ:™Á•a%µÀ;¼,k˜Õ@VK˅yý@Û{Òv?»4‹"'Å¿º¦ƒŒçÚo@Aâ"Ÿ@†Õ/ò¶ì¿Í™—@MøÜ¿éoÜfÃË¿í—Ù¥ù#m¿Ö
‡­ÞÊü¿¥K鞥Ù)¿ïÿ•ÂûAGNbcuNVSS J193349-102530?ì¯ôïI Q?¶ŠÐꙞ?"ø"Þ¬x?½g6ÇèÈ?·áGéðÇÜ?µÔ÷"Ú?í¢"Ɔ"?ÀF'Çc?t£¸ö÷ž?•¯oçì%?±¤´Jj¬f?¿ÍݤîÂì?és–ÿƒLª?¬È=4|ç
?Ž|<Ýh-š?'/XÕ:"?ÈIà4J}?«n1	Ô/*?çª]ªäę?¶G°¹û€¡?c,ęr?câ1C*´G?Єë¬í›?¶š8f^4FGL J1934.2+6002¿çøÐòSøƒ@25Ôèû½À:ç|ò™åðÀ<«Þ7X\@ uҕ¹/?ýo"èbT‰?Á¾BuE|?ÍD<ÅÙ«@Ã$­^r?ù(ǬÒ['¿ï}'›x—?ïÿ˜k¥k?§ÿÚýMY`¿Þ)¡"I¦<¿å?4(%¸÷¿á9âyÝ;°AGNbcu3FGL J1934.2+6002GALEXASC J193419.64+600139.5?î©ÎœJz|?›ÙéhÞ}©?˜´2=ñê<?"±µú³kã?'ú8¾Æ/?ŒyÉÚ‰?æ+T£e5¥?ÇZÙ[µ®?ŤQÁc?ÄVÃìò"‰?Â;	!Wh?´ÊîHj{÷?ë|Ó>pï'?¥t"³%C?®Á'T÷($? }«ÌË?´¸¤áüò®?–'g'WÎ?âà¼S‰ž?®…ÓIa¼h?Ǹ?÷ÉI?°
¾ž>4?ÌÄμ8>?§NX¥ß]…4FGL J1934.3-2419¿èÏmͧ¬ñÀ3Ìu_þmYÀ:¸£a™xÀ<psT‹r@!	L;P?ùiU~·–?Ë!Õþ#ÜÔ?Ò7A_ƺ@к%*\@U'•ñ‡¿ïÛ>ê÷Z??ïù> #Ìc?ãÇ¡A(¿¿ØáŸÂ¨†œ¿ãǂÀºí¿Ù‹n]«¬ÂAGNbcuNVSS J193412-241922?ï3YØ_÷?"m\ü%HÂ?m—·[*ê?dA<¶¡ß?›ÆÙŽ£Ñ?'MWÎ|	b?îö-5
ó;?Ðuù2†?l;$U¾ƒ?'ùoT¹?²ôÓéÈQ?™£DËÕRl?ì½ÍX&ñ?(9`¦.?•:mÈ>?˜êN!,ë?¶ô·z¾Â?™â•æµð?ëµÊö¦ª?¢r4k?‰ õ‹"9y?|¸p‰-'ü?¿-‰™Y›Š?¡wÈ\ßS4FGL J1934.3+6541¿ïÿœF-r@4RmzVÞ3À9ËÆ<ÓGÀ<J<Q†Û@ߝâ)@/¸¿Þ¨?¸öç?Â,ñ$ÅÝ@¬ž#lÓ@[µ³U­¿Å\ÿµW¿èOÉkï<¿é³^™‹¿î‹1¬Jv¿ïò<'Î{#¿È³çcQAGNfsrqTXS 1933+655?ïû"O«x?Mî{ÝÏ'?6ö"¡®ûÑ?AuYpG§'?0EBàõ@r?C''ÄX?ï´ÎÇ¥F?ˆÅŸ1Ä8ý?Gk²M×çÇ?_Ý}o	?U'ñÛoç?‡XZÎ@â?îjI~ì8M?—·'I8?zòùˆd•?vϚù½zy?¥ýà/ús?—;Şå–?ïóº'àÉv?G}åà:W?2xh"•?&©f8%w¹?SìÛdh-Ú?EʯQÁ5ô4FGL J1934.5+6139?ånãM Ot@2Í=B€®À;hIóiÈÀ<¾ÀÕGő@S>€ï(Â@è"»ìª¹?Ñ*—ëè?Ívñä^cã?ü4#óûÿ@æüõ‰"¿ïý–Þÿ)k?ïÿËô_¹¿Ú#½l²†¿è}}`ݐ¿Ú)À£s¸	¿ïÿG=¬2ùAGNfsrqGB6 J1934+6138?Ù€"?}ëˆ1á#?aÊÏÓü!?YÒr1eW?ƒç•Ã פ?{Ä
L&2?ïSŜ?%8?'l€'I)?X1ŽCdÓh?eL K¾·,?"3"å?wæý½?ít¬,^v?—,ÑÄ"zM?c#:É¡?'»H§YQ9?°AÕضYï?'}àÊ5?îÌ[âkk–?‰¿4ª€è?uåÛ	ø?lW÷èËS? }Ÿ=è'?‰ˆÇaöWì4FGL J1936.9-4720?ècTvsáÀ;ޜ)¦À9¦óp.À<
—þ@ ¯K¿F&€?ûé{DD?±¿jŽ",ó?¡¥ÓÂ=v?ò¦ç•¥ï@œO3™àf?ï{ˆA'¿¾Öh¬çª¿áJÕù¿Ô~Àdß}©¿ÝÊhÙÞ-G¿ÑÛR6-¹wAGNbll3FGL J1936.9-4719PMN J1936-4719?ïé^†µ!?Uà.·å‹™?*ô×pOÓ? L8÷†?dò+Ú§áÄ?TúøÆw>ú?ïÅ®mQ•?ÑÍXˆž»?/…çĤl?DѬ؋¶
?|,Ћ27?~Ê©Â0‰?ïI~ù=á?ƒU‡^¡ì?e…]uYÑ?TŒ"IÊE?œ†.5)˜¸?'¨[PÄ@?ï]í_‰?vЅðŽ?UÍàÇ8̉?C&ìßèD?'åoç›Ra?v3ÑÐ?÷4FGL J1937.0+8354¿ïñR\]î@9ÄdE#öÀ:úôàM/À<Ì+
|À@ð?S	?ÿ"Ñ‹xn§?Ċî[ôt?Á·ƒåRT·?õA›«Â'@œ¶×Âõ?ï§W\Þ'h¿àÓC>C1®¿Ò8¢]ã`¿ÞpGüó¿ägûnj,¿çã¡àø0AGNbcu3FGL J1935.5+83556C B194425+834912?ïCÒÞ+J™?‹f²ë@ï…?n	œ¹ÁˆÍ?d>m!ۚ?"Äp£^{±?‰0¨?wÞW?î"Öm&??™þ{WfØA?rΡtŸÏ?vÉò¼úÝI?¤Z'Z¯?—€î…߃?íó 1ób?'g9•C?w턟°¶?eÀëk¥\?­ÐF™³¾?ZӞþ|Æ?ì—HÛ¶?–—2ÙÑ%÷?˜ŒSÃô™?}ܝ&«˜?µ"ªBqRk?–`Þ5l:a4FGL J1937.2-3958?á6M}r'»À9]&ú?̟À99­feÀ;ÿ<ñøÖ@@8xž!h°@è÷QÕ?±‹è.ú?²n¶l
Da?úÔní¥,@ͲûÀU¿Æ‹&ú•²Ú¿ä_ÿD]Å¿èØ^›–ÉÜ¿æö)	€¿îH' XÐ|¿ïµ*Ÿû AGNfsrq3FGL J1937.0-3956PKS 1933-400?ïÅík_N?ypЯf†?U¼^Øï4?S~Iº>Cá?wš\""*?vcoÀû§?ï®±ë<5È?‰dÁö?HožQú?aój†ÿ^Ÿ?'Ò7ó?†)xËWü'?ï/ÛNÍ1?€Ç-كø–?rg™·_<Ž?g6ñ¬¹07?•…Þ(NŠÍ?|NXìC?ï£a
…îæ?qNŸ3ù?p˜3o«æ?a@ rEû†?~1á	˜á?gîœb|<A4FGL J1937.2-4217?¸–p±
QýÀ9óôým~‰À:ŒÆˆåí/À<pŠ:N@Mš{õá?ÿ ö4¥#;?Æ'7RQ±?ֱñðþ@
U°†E(ÿ?ø6+|s?ïsþÕ]•¿àñ
™¶õË¿ØŸ"ðoê¿æ¿ÞNÕP¿ëV&x¡Q¿ðAGNbcu3FGL J1936.6-4215PKS 1934-423?âtS¹7¥õ?ÁfŒe?¼2–ך?°…=$á?Ô
§çÚ͓?À©•?oZ?ä« ÏU?ÇÁ6fj¼Š?ōsì™?Ã]†Bin?Çh@rpÖ?»h,A:òH?áûL
FÇj?³J"ÖG?ËÝÆZ¡3B?¬Â«õ™?Ì5	pC¯?©¼9'ð?ÞÃt1ôj?¨'!w1kÆ?ÇrT"øÆ?¦©"2ƒM?ՃÔC"2?©–žX<5B4FGL J1939.5-1525?âv#‡05À1säXÍÀ:l`´u½òÀ<ŠJq=Z@¹UÐ-@ò…fîW?ȳ¤‡´??ÈÛؘÝÜê?þ06(°ù2@/~UñN6?ïá8ÿûÎB¿Ã
3µŒ¿ã% ¶Xí¿ê(ƒ¬ÈJ‡¿Þ.û–
óß¿ïÿÿ" 5•AGNfsrqPKS 1936-15?ïûQèm?–LÖ8ï ?Us0?q\ò?Ç°Ö?xáUb8?'&Bþ&é?ï¬a…Å?‰¯†i(î˜?@lX`aZ?_xuå\$?ƒàôuø¡?‡UûËÕWš?í¬ þÏý?—Vµ:cn©?ˆ@h)àÖ?~c=‰'0?¯%äÕÌî?""ß±Aë?ï y´½ÝV?xÌä‹?[YoG×@?L"k°oÔ?š;1QO×¾?~­¹öàGG4FGL J1939.8-4928¿ïu‹%@âÀ;äÿëJwÀ:…¯	ëÀ<ƒ€Íù¦@þ£NÏ@~â¡Jh?À(ÁÕ¢ß>?¤3Ê7-?怮¡=§Ö@¬¶`?ïØ5jÀ¿å+îÑ"2¿ç$aß(ì¿ÐÕbÈw(¿äÆ>QÊM¿â™ДØjAGNbcu3FGL J1939.6-4925SUMSS J193946-492539?ï´Öñ`š?~rtïݟº?C-ø‰Ån?5· 
Ñj?—djŒû?}ã‡ÈŠ°?ïnK»?''Ø~wU©?Dóp-þ›?bl;\a?'jߥ!?'-kñ`\*?î»oèåÓ³?ˆÛ€qfó¥?jÒ¢¾°?WÈLí'?¢›ßñx˜û?‡edôŸßÑ?îèÝk4<#?	N^q)]?m£^ðXÉ?W}êgŠ$h?Ÿ/æÖ:p~?€3xd"G}4FGL J1941.3-6210?­›H4;	ÛÀ=‹*{ԌµÀ8	j#ŠHÄÀ;½G²Jk@ÚN#yÌ@͝€Ú†?—ËÄLJ±?±­­ê‰@»Šãq*@hŸô|"%¿Ä|1>fm¿â΍âVKç¿æK<>t°¿å{f¾%7¿è-••¿ì®Ö­ _AGNbll3FGL J1941.2-6210PKS 1936-623?"")æ?ƒõ'êˆÀ'?Xpön&WÅ?R«Šîâ!z?†E<i°»e?ƒ2ßE/5O?ïÀzž×+?Ø/X²Ð?6ޜûÀ>1?NRm%bV/?~UàØfw?*û®‹)?ï[sºÒ¥?~'¦
7ñD?nzÛÞ$@?b¬g¥?Î¶á#0?zR¶Mèb?ïúü÷‹=?5h¼­'[¶?Ne5¡…ù?
·aPäk?A"U,W½a?3oEé5ÿ4FGL J1941.7+7218¿êwìwPÞ.@6©£Ò؀À:J¤ˆàä²À<¢—o@Í Øè@|lb(ê?È°`¢|?É2ØÅS†»?þ0¨ú_­@Ÿè)Ê~¿?î¼#Òm¾¿çk6#¨|¿èÏa!Xi¿ìn	"&¸Ñ¿ÔÅ
á…k¿ïÿ]þ¸Ø#AGNbcu3FGL J1941.8+7218GB6 J1941+7221?ï՗	št?wtJ:lé?`Ôð®9¢í?iŒ™?i"þH+èˆ?n,ļ'êå?ïrE¢@DD?"Ã%½j?VE+(êǔ?jß#Ž,´?RùhÊý?'è¿,?í#Ë'ُ?œ•	Qo®—?"'¬£´§"?‰vh±)}?±ý<"	«?–rSÜ8-?Ñ/¨è?sãÅ]>Ë­?Ni±j0?Bf1 tŸÿ?‹3»ª¯=?s˜¶?Ð4FGL J1942.1+4011?Îhüe85s@ ¯'Àa"À:¥]òú^À<^úaZŽ@µÈNbä@õ‹$‹Ðƒ?Á7ÉðÏ`?¼2^½¶Á?úƦå²@IÊS˯?îOd1¿Ôʍ'_d¿ã?Èl뻥¿Þ°¾ä¬½c¿îÈi[
lÐ?ØÕÔ]dßÿAGNbcu87GB 194033.4+400351?ì¸ÞÏó3•?°T'ø'b?t×A<S0?põhòX%O?¸ë•l¡0[?°ºâ87}?ìßVӇÖä?¹•æ0€7ì?aˆ"²åmE?;éwź?¸y¾*x?¹@RDg#G?ìW™Èc?ŸNêlÛå?›®"'¿?DhLe¹?¶WµÙ3 æ?™6"tQ‡?î§Ê֑?" k¾Ä¿?yʅp¤ý¼?f~ӀÍ?¢JQ]÷:?'Ÿ' ™üÌ4FGL J1942.5-5827?ì-"J
nÀ=rˆXÿu—À:ÆGœvìÀ<'§4ŒÏ‡@ü HtãØ@D¯ñ¥Ê?ÈA¡µòÁ?¨ÆÍYd >?áz`ƒÎV:@¨L!Á›Á¿áë¶!d©£¿è¹> #Ìc¿àŧ߭z!¿×šFÓ#(#¿è?`Ónu¿ïÿÉ¿&FAGNbcuSUMSS J194224-582824?ï¢ÂWñÖ?‹¹$Õòæ?N¯qP¦]'?D-cblž?…drî€Y?‹VŽv¢.0?ïvf‡ûÕ?""ç!TìZ?<˜RŒBÝ?M-9ÇÔ?ÍqäÏzE?"_ìZ¾g¿?îQ1¾Ký?‹0Ãú;Þ^?w†áŒ|v?k³YZõN;?§ýд)°"?ˆÏ¶ÄfÞ;?ïJŠ'r?xÚ­Åïöƒ?aØqXê>ö?O,"Åx0?"sŸÂ"uÒ?xFêõ°z4FGL J1942.7+1033¿ÛÀN~'Àsºc=¼úÀ8'%³ïáÀ;\Ì.A\@ K媔=º?ýWo£&
V?¡D{@N_ñ?ž@}@¢?ý™œô˜@֛Ž¼Eì?à@%‰ýDd¿ÓošÂŽ…i¿ß¢Š# ï¿Øae?õ¹U¿Þߟ!î½8¿×Õó¼ûžqAGNbll3FGL J1942.7+103387GB 194024.3+102612?íê®Æ›d»?¡9ë-ø·Ñ?MAM"÷®?E‡Çì¤Dñ?°p0å²;?¡!6VIK'?ìŠÆ€3?¿•±èÚD?DopéÜX=?_Ðv覻?¿ÆdÇøEÁ?¿Šb"ƒ½?ìC/҄´‰?¢¾éßh?€¡à–£?sw­ä»a?»ÒEYëÕ?¡ìªÙ7©î?í²½™2S˜?–«(gÕs?zK?Ô%û?hôî'á·?°ÅaRp å?•y|¸lk4FGL J1942.8-3512¿Â"/&–îÀ9!zg¥*ÇÀ:˜£ÇðÄúÀ<7β€m@ôÃ@Z±'Ýãv?Æ-Èe4L?£"k­"8?ÞÜþ3!@@
2žb×?çQj‹¿ß]Ò®Že¿æjußÖó¿Þe¥
æãϿ֘…·d†¿ìƒ<àÛødAGNbll3FGL J1943.2-35101RXS J194306.8-351001?í3ÆwìÍ?¨àü+R;?cR»¥»®Ê?T5 ßɒ?µÇ6ckº.?¨¢¬(Ä~é?ïpsԌÕ?ŠÇ"œìD?CQ4(ˆeº?T^xZ©Ô?'cgä*"7?‰tzòttð?íX4Jˆö?šADþZF?xWAu&Ï{?eŸåº¡v·?³ºZFYK[?˜¨£Íc
T?î=}ó£¤?ƒ˜®l¡=j?_«;‡HLU?N÷ÿŠï«¨?«*Æé‹}R?ƒxë]`n44FGL J1944.0+2117?֎{׊s¿õ
WqÖÝÀ9Ÿ©,£ÍÀ;¦I†[Ï@#Lo'*;h?ô…UÅ.rÚ?Á`Ü8Ё?Î雥"c@Û£)eT@~¿[5z¿ëgÑÀ§zƒ¿ïé†@÷A?ì~ò¹Æ_Ë?ïýßÿ¯x(¿ÆØB¡»&¿ÎÅͪAGNbcuMG2 J194359+2118?àRž­ò›?̼³¨)7?£·[Ò.¶?³åJ(f)?Üã×+ŒYò?̇W£™o?ßÒÐcT~?ÔT(àP<?wÔc|15?¥€™77)Ô?ßÍލæ¯?Ô/'ŽEÕç?â]ý¥Öv?²†Åw$Ÿ?±ýP/"X?ž¹µ¾Óª]?Öä`Góþ?°Öó,ŸW?çüêJ³Ÿ(?ÀÛö¤w'?{FEØq^?'Òí¬ÙL?Ï2$¦mû?Àë_Rb¹¨4FGL J1944.2+3921¿Òâg–ð¥x@V#ˆÀ:5ƒO«8þÀ<+øàQ@>c†ã£?þG.¬?ÀyF¨Zý}?͐ÉE.@ßkã}é:@%ˆà%?ï¨ÙÞ-Ga¿Ô¿·%Á¢¿Û7'"Yœ)¿Ù ºKâ¿ç0²ð'´{¿è֔aKtsAGNbcu3FGL J1944.1+391987GB 194223.9+391242?à]€'«£?ÀŽÊ4tÿ'?º<£`Ñ؏?­¾d§Ž`ó?صÖØtB¿?¾‡ˆÄ>?×*ª^ky_?Ƽ›Œ(rŠ?¯
ö¼?Ž'?°‡ØÊmÈâ?âyûeJh?ÅoIhæ?æþnOèr2?¬Âñgq&}?³Í¥
Îfð?ŸÊQó1ìß?Êt9w¿?¥k5ø3'?䀳É.Ó4?¡2ÛÀ
»?´.…tÕ

?'lðuþÐ?Ñò÷m? À†×?;™4FGL J1944.4-4523¿Äî'VSk.À;ãü–þµÀ:òŸÅ,ÅÀ<aV"@!±ð°.\?øœ5Ċß?ÃoKè5Þß?À¤AhU(ü@³;–¯Ž@K-Kè‹Å?ê9!°:?ïÎ~T–Z¿ß€ aIq
¿È"CÄOû–¿Éö$_ó/¿ÓóBWhrAGNbcu3FGL J1944.1-4523SUMSS J194422-452333?î®9gY? è3Ûçú?fÙ&è'ÝÞ?a/7j?£±©û@*? ¬€mqG,?ïjYç~¸Ä?ØmÄÚn?KйÌtúA?`{n×Ö:?'Ö=AÅ?"?2@B}—?í
þug?›­øúUÝÔ?s—ªÞ›
?_v"¼¤0?¶V'¥£
Ê?›7ŠF]«@?í-?Œh8Ò?šrË;5Cß?y¢5YA‹?p}Í ?°ù?´ûàG* Æ?š4èÁü>4FGL J1944.9-2143?îÀéx:_‰À5ȊGìÿÀ9:._ŽÛÐÀ;݉à¾ò@ di¾µ‡â?üYÝÁç–?®JícÙª?«>Ÿ'ª?ÿÛÇ4Ý@y؜ŽÁy?ïíj Ûç¿Ñ*Ÿµg€¿Ùêã"ύǿԠº $x/¿á`‰þ#r¿Òr¬ÅÆHNAGNbcu1RXS J194455.3-214318?ïùˆ½S	.?>séì¦?™1Ü?ö?À¼[<!Ñ?GÉä'ßÂ?<–±Ã­Ñ?ïÎV¶Ê"*?|v9*"4‹?/·4ËNr?FôÍD‹?wÖêô"zá?{?ùúÍt?îïF­ÑÖ?…«ì([Ã?kE•™?bŒÇ˜gLÑ?ž®›¸3#R?ƒ§Ê¬¾‡Å?ïx #<?t°Ì•r`?Q…²&i:\?A²k7|?§C2o	¦?tH§^¨4FGL J1945.1-4007?ÒpöŸ{}FÀ:Þ*<êlÀ; κÖ¨À<¾€íÑ)S@éé%Lk?ÿ^½çX?ÑÑT›ã Ï?àùJn¹?@ê¢þ)q@
u?Öڗ¼¿ïÿÐ?sŠ?ïýáAÎ×i¿À¸™¹úã¿â–Æ ¸Ç²¿ïÿo·HJ?ïçh5'‰AGNbcuAT20G J194519-400557?ï";pXLÂ?‡ûNïÓãs?XjÛ·*	?'§õf3â3?s1rkJÇ?t™eÕãÊ?îêM'À²?£Îœ5ÿh?p·‰ž«uv?ƒ҂çSÎ?žŽ3çýŽ? ³éê­2«?éÐé³þÔÁ?¨ÔDYÁ$?·é×/÷0? Å­Ÿ—?ºpȈÙbÄ?ž ̱¥?ïRµîFÄÐ?€3&ÄݲK?rÿñk Y–?c)ÒÇY?éEÜ?O"?|f1y$¶ø4FGL J1945.5-0153?ï*[¾ö(À)È
°ö­À;!C|V'´À<9.¿0@>ßôñ"@ݼfM;ó?Õÿ\÷§Â?âQýŽ5¸I@mczù›b@ÔQpµõ›¿íسà¢ý?ïÿÔqܼ¿¿‰c˒¿êDm'ºZ¿ïýibDBпàÇA<á1ßAGNbcuPMN J1945-0153?ìàŠëÂ?±\a·YFm?±ÉJÜy?­±ËJAIk?ŸÐ·†#?ÀªýÂ?èÏdmgž
?Ä%‹ºúIñ?»êèS÷?¼Æ."‹a¯?½šÍ¬o¤?·UÔ¥(	Š?ä†[Ù\T?³Göѕ£¿?ÄÑÔþìÆÕ?¨7é͞–b?Éّ­ÇÚ?ªpµ§6?æ|ö_5í»?­ü݄"L?Ãڇö?¬­
º…f%?Â1Ÿp25?¨(©#B`4FGL J1946.0-3112¿ìõbÅÇõÍÀ8'ÿ.Hè§À9wQŸ/ÐÀ<	ûï»@r*$Þä@•a[dª¥?²&rÛiȜ?ƒNcnÝÙ?ѧé=›Áè@#â~å¹-?À~Õ]•¿éýaw¿ámÔº.¿Ùˆdà
—¿é:aûš°¿à;š{pdAGNbll3FGL J1945.9-3115PKS 1942-313?îPˉíþ?¢\3¶t=?{-˕Äu?sv5!²Ñ?§˜yÔ¨'ƒ? øàX}žT?ïnë_¸M?ñÁßôú?N34œ‰?d&ëw¯L.?'0û÷U^?ÁñßB»¦?í^ûµe´¡?œ"ôÆO?…""á:(?{²a/¼?²U'¸±Ó²?˜è²\'è?lo\?‹ÇTÆzg?}¦¶#¿¬s?h»ÚOŸÒd?£é`dÁ¦?ˆOÀ'V4FGL J1946.0+0937¿èh£Ì'./Àõ@‰]À:Ucé´d À<DF€íÑ@ D§•ßc@ÚõýG¾Û?Áò¦%C0?ˆäŒ1&=¬?ȪJè\@O7 «1¿îAÎj[¾?êÞæu¿ãŸD(y¿Ù]$~£²¿ã·/+H¿â(TÐAGNbcu87GB 194328.9+092856?幄[På?¿)F5ˆêÔ?€jê|ú
?r£øÚúáR?Ô	ŸøúMù?¿âǺø?äå2ŽqV?Ç@Ymr?Xý©ö)Nz?kèðü2F•?ÖžDìô	?Ç/
(liO?çI?áŸ?«²'tnçu?—ïªÌ±åA?ªÀ¢f3?ÏÝZãFá?©ª*7|Y?ê¾ø!ݎy?œ]
ý²k±?¿Cé÷?xôÔa˜ˆ'?Âì6ûiƒ¼?šÑža€¶›4FGL J1948.3+1207?ïùõdúMÀ.Ü ý¦‰À:ˆ­Ú™>*À;ô"ªlO´@±)bNÿ—@=sãýjú?҉Uê`o?æ
²
©§@/'…€!@BZœ¿ê?é£%¿,P@¿ã÷æV
ΐ¿àüÈþau¿êèNòÄ®¿í¦i³Ê¿ïÿâ–é¼AGNbcuNVSS J194814+120645?ÆÐê Aûù?¹ë•óïÖ3?ÄJéN[ú…?½Ï¶JLgè?å9$X'`?ÂȋCÓ!V?Ô5Œ¬ðx?ÊWp±ÿÂÉ?¹;17ù¡?»"ÛˆT'Þ?â½Ùc؈'?ÌMò ¥ž?Üïé‹^g¹?³`ù€Üu?Ìæ»ãç«?¯ÍMÄ!¹?ԝ–¯¤q?¬¬é"sYp?Ø8§.ßG?ªšÅ°'ï?ÆêB91Þ?§2oÏà·?ܾcO´‡É?®ó:¢Ùå4FGL J1949.0+1314?Ý$T¶zÀt/è%çÀ9nç¼<[ÑÀ;˜Çÿ²|@`M"ÃÌ@ïÃqÚ7ï?ºþy×ÝL?¾eà¦@æ<$s|Ï@›®] ïú?ìö쀜GŸ¿ãÿ!é^ÓË¿ãtßp=½¿çIH¾H¦¿äé0&Ž¿è¥
±3êAGNbcu3FGL J1949.0+131287GB 194635.4+130713?ܱ¹ÚÉ_Q?ÁwˆlÝÝ?"×^^<m¨?¡ô«ØG?áh©lë?ÁØn?=֗?Ü&Çøwÿ?Ç¢–x†ý?"8‰ù›¶Ù?›¢"­Í'y?áR׳÷žJ?Ǩ•ã"?ãðR™{?³FŒfÑÞ±?¤ÌXöm?‹¼,:æ?ՅÙ/®Fð?±ëƒùÆ'?äv¼ñš?¡R]Œ§¹)?°'˜ó¡Š&?Bj8`"?Òó"I4iI? Ó2ù®´4FGL J1949.4+1247?ç%³HAbKÀ©Oð\À:‹n}ŒÙÀ;¹rl.'@ŸœBk_u@gFBÐ_?Ð1Ñß0Q¬?ÂÊ7F=Q?ô‹Ëz½5€@®¡É=÷¿ïü2¶5±"?ïûçÂq¿ä¡>iÈ¿âÄî|Iýz¿å±[Ývh<¿ïþñ­VåÀAGNbcuTXS 1947+126?ï(Ñßc?'‡`²ÿš?Z¶q%ÿ‡?XkN"œpà?™Cà
Óª?ò˜'Nü ?éüáq~3¡?Åt¯¢µ?Mº1è@"G?hMt¦iÅ?ÇîÀñY?ÅNUº»a?éGm3îìm?¨`îIˆ ?'‹r'#^?éèdâ?ȐÜÞâ†?§
$üªU{?í5Bې&7?˜)Ê¥´"1?k"ýüˆ¤¶?_+ÂbpDK?µyÁ3š‰&?—û·)=4FGL J1949.5+7311?Áùœ…ÿ€@5ÕU>öµÔÀ:WçG¢VÀ<݂ýuâ@Ÿî)†Œ@͒tâ*,?®Ãaéÿã?¿Ú®ó׏?üØþÒ—@Nޞ†hd¿ß¿1×JÕ¿æêG1ù¿ç`N‰Ðκ¿çXjû ¿ïÿÏ=ÀTï¿â"h\૧AGNbcuCRATES J195016+731028?ïŠQÓj?ƒøh¥îõ'?xi°Æsu?xÕfð!Ù?G 2ÂEÊ?zs\ɺ»é?Ë'¹?¡nN!:^Ø?€¬ÕêQ}?'"Ík!?£qè	Ò¦?™Ù¤‡ëô|?î~:.HJ?Ž ØC_?€˜ø?'w^?r
Zþ?£ö±€L?Š}|è-?íPbðxK?'·Ø¥êe?™hY)Ÿ?']yˆ~C?®E¤k\në?Žï<"c4FGL J1949.5+0906¿èæ=öÔÀ!? §?uÀ9·
Ø/×^À;ýžvx,@ X醖Ý}@€©Þ‹;?¶"ÁI–¢¿wä
¨‹R?Â
]v'Ï}@
$ô)Ýôè¿Ô"mè2Ú¿æô¸Œ£è¿çÏ
Ÿ$óÕ¿ÍHuûìÊ¿Ýqœ¥g®¿ã=ȝ"#^AGNbll2FGL J1949.9+09071RXS J194934.1+090655?îéù]~šþ?˜¼úœMµš?JÉxäV0£?Bò,&[£? õDD"÷Y?˜_¢–cìÜ?ìëŸËš"?¼ˆ©Â²Ï?8ËW!^W?R¿±ó?¿Ç×çL
'?¼tâ^6šG?ítÝ$ID?˜Ôc`x?ud9%3?a1ᔇo9?³Ó䊄d?—9=ØÂVÜ?îÁ*#NDÉ?…à=ÝÐÃ?\±ïªoÍ?Kerz­Û?£ÎRÖ_÷?…ž|ugÆÏ4FGL J1950.6+3456?×ô¨ë#Ø@&!`¢ØÀ:±îX7ÏzÀ<.ʔ
hž@!P¯ýˆ¬?üâDhå?Ó«'Ëöãø?ÁP±ˆÎ›.?÷X¨ø².?ÿG˜ÛX«¾¿ïþ9áùâ?ëa±Ë¿†"?ïü¾A™¨]¿ç(Îàù)¢?˜!ìf#¿éßÓÚÞˆAGNbcu2MASS J19502776+3456224?âŒÌùÑJÔ?Äý*"¿«'?mç8óu?d¢#8¼˜:?Úª–Ñë"S?Äîó'»¶?äO|ýŠº?ËXÖ¢3:¹?t]ëd%g,?ˆëqì.'?×{éXtTð?Ë¿KºÝƒ?çTn'•Ó?©ˆÿ÷XÅ?•µr÷z'Š?€j>­Uä?Ï÷—–¼zˆ?¨'ÙZ*œ?ë»Ù'úëh?¬É3ƒ)Š?oòÚM¼"?uk¶_Äò?ÀÎŠßßh?¬±z¢§Fê4FGL J1950.8+1211?íFï‹Ã&À!úvSCtÀ:دYÀ;ȟ·ÀÌ@,Ža'&@û
z<A?Æjt!?݂Bdÿ^@ítýØÞS@°7êê¿é°ò¡G¸Ñ?í˜{V¸sy¿ä–ù¬(è¿ç(ÒÁ&¦¿ïÿMéDÓ¿ãÒ ß²CAGNbcu3FGL J1950.2+1215NVSS J195059+121316?±38ˆwè?¤'Ø&Q¤×?䆨_K?Æ36Ù@œ?Ò¥àß#§Þ?đ2>Uéä?»¶îÀ]R|?ºí¾ãÂ?ÝD£Ü@º?ÍI"ÈîÞ?ÛͶ¬j§?Í0ï5£Æ4?Ârè.â·?¡ªàî0 ¶?ß©Ìl+…¥?³!&s†ø}?×Mú½ÿ?¯«¹¹¢4?Ìⵘ"?¥¹®¶?Þñ:"?´QŒ[-?Ó3ݜù#¿?­£àhÝ4FGL J1951.8-0511¿éÌøPߥÀ/–¤D‡À:Mqåöi~À<¢Ô«¾_@܁Ðz+@)2^!‡?Ç*ÖØ¿IW?ʘD/ùŠ@¼]\Òi@8lýv?ïö¶^Ì>¿®^‹{ž±Ü¿ä«¤=âc¸¿ã_Cý…Ò<¿ì]2K­¿ÏÛ¨ï³AGNfsrqPMN J1951-0509? ŒºŒ?›B°©½?'…ñB†ä?z#þî÷O6?¢³Yµãµ}?˜¡Ñ'¬b?ïl¿o*ø˜?"Ë™R>¬(?W7tÛâ?nS'âäÄ?ôšÒïb?'µË—ÊT?ìÏNƒ³? fъ>À?—V©ÞˆÚ?‰> ÁXé•?³±»Á¾,?š3E‰—É?î!iœ??Œqˆι'?vµejÀ°?`k6¤\Ç?«Â<(ä?‹m†>R®"4FGL J1953.0+7651¿æ0ª}þ™µ@6øäd™ÍÀ;TÍ
à-ÓÀ<±
?x@k w™¿"@pðÀÇÛÌ?ÐÙÖÀÁ{¶?̓{~% ?ø‰Z¼äø=@ã…"¿¶?Äßbцp?æ
ÇNފ¿ãxÔ'4!¿ÛŸ¯È°š¿ìô_î} ½¿­s£æ¤AGNbcu3FGL J1953.4+7653WN B1955.4+7642?êm€}±`Y?·2R"xÖP?§ÈÉÐPŽ?œá~xˆs?À‰ÖÆjy?´ûJ}?îÁ"²Õ?¡¤¦ÌKM?"»~-×?†ãÑs°i%?©ô[?
2?ž'ŸeX?ìVð¤A©?¢õ?¶)?ŸŸbI?Œt$
ÀH?¸à¢X`t?œUgBèÅE?ëãÞ3i<¢?šºˆ²é!µ? †à‡\,—?‰6ïóɇ'?¸ž!¤?™°ô<ëh4FGL J1953.0-7025¿Çw"×°"À>–Œi/nƒÀ:PYddIÀ<eî \+z@îl"¸Œ@vg=%û<?³ÆÊ¿¬RÚ¿©§Çà	k?õÓ	AÈ!l@õdW"¿ãc¸6<Òï¿Õ'šCÅ
¿æŸ¤¯rÊ¿Þ½Ÿ
ò¢¿ãžlґ1ì¿Ø<åcœˆAGNbcuPKS 1947-705?î,–®"z?¢ûmLZî;?q?ÑÝÎ6?dtQZ"{u?«šÛ&"­?¢=Ú«2…?îw•¦Añì?ª¼:7ËxÃ?a.ÙPŠÂ?pÛbOz?§tâ®K؎?ªï¾¥%?í*Ñ>Ùd?™¨P?|Ž?ƒË¬}ŒD¥?sK©gÎéM?´0~W¬M?–ý²ó}M?íE{¡à?'ìUŽ·yP?Š;m
+®\?uæ°.‡ä?²	ŠÝ{@?'Š^™‰K4FGL J1954.6-1122¿Æó7kb_ØÀ3 é_ªŠƒÀ8çDŽ¥JÀ;Õ¤xð¬¦@›jT1°@YgåÂg?ª—Àâ™ú?®¬Bn~R@±!«KrÅ@¨sÿ¬*¿Ã£]<Ç¿ä%"?]ä¿çšÁaߙ¿ã(ÛPN¿çd×Oݍå¿éÅW ºJAGNbll3FGL J1954.8-1122TXS 1951-115?ïâü•Òæ?gG©¿Qž?4³u²õ~E?0nÄb¼»?jm³ÎjŠ?fŒeÚ?vu?ï×qv™‡é?xIW´l\È?1(¡1Õb?FIðÊM¥=?s4º º
?wµ±Û¿¿?ïêd<M?ƒëm™ó?nKӆÓ(?b'à ä?˜YOÞ
¼?8Ûÿ-u©?ïÛ{SäÝ?Yв+Z§:?D%1ï€óG?3O†>³¢?o{$0:ç,?Wæ0XÏ÷ò4FGL J1954.9-5640¿À—ÁÄVÀ>ütÙÆ°SÀ: ó9H *À<`Ñ>K•*@ mIT1Ûo?ÿ*.!{zË?²yOa½	`¿¢kÁo Ÿ2?ñh'iIo¶@RÉÑoÊ?ïقˆŸ¿ÕŠûœ$¿åÕ¶`#× ¿Ú_á§Oe¿×LÕ[;ºì¿Ñ¿LF)¯ýAGNbll3FGL J1954.9-56401RXS J195503.1-564031?í¦ãËGå"?¬–¶Öå?ph]¨c€Ü?n´$7Ν?±Â[Ë:›b?«i"…X¿?/ÿ=?™«]Ô¯CJ?TmƒQ¡Wé?_fòa;9?¦"æÍ?˜Úüä¥DÇ?ìþ^´é¼È?˜#cñ	/?E `ÐY?p"2e],æ?µäfL˜"?–Ôš.Šu»?í)E	S?"&IŸf?†ÔÃ!õ2I?s'eÂÓ]7?³Ý/)™'?"gbš¹é4FGL J1955.1-1604?ïþY().À5%ð=]…À9¨èÄ3¡À<MjìÝä@ 2ót'Ý@8S 8"¬?²¼ùÅÿ(??_£Ê­à—?²~9|§›@éú8•Èª?ïoAT©P¿çPB7²ô´¿âI>¢Òþ?¿àÂkµZÀ@¿ßì.Ý
6Ê¿Éæf%ù¹ÀAGNbll3FGL J1955.0-16051RXS J195500.6-160328?ï螶''Å?a/ŽOÿ?17Ì:ž4ï?,‹ƒES?e:PQ"u¸?`_¾]ȓx?ïÀò=ç‡$?€²ª×J?*·'¡Òœ?=^ÜN˜|?~±$÷-Þ6?€N$°³*Å?îÁ+ËaB?Šý+ì=ã?nø^|)d?k"g&1ý?¡ýÈë‡Zß?‰ò?Ì`ù?î¾Y%À}?"Öormð ?jíÄ#Sç?W¤€)!‡?¢pÞ+nÇÀ?"sÏLöê4FGL J1955.2+1358¿éÙº©è#ôÀAÞÑ·À9å½^šÀÀ;¶UNæíà@ÂІ×}@6ï›-îP?¸_ðU"?ÇhóÉæ¾f@
'¾}~°à@¸Wï«&?­3!8E'¿äŒKÓ=)V¿ä$"Ÿ^Õx¿æö`y½[@¿éœ#î¡¿áüŒéAGNfsrq3FGL J1955.1+135787GB 195252.4+135009?í8¡ÿ‡9?¦¿ÙºGé?‡^úAÊþ??ö3J(Ã?³O»Žm?¤Æà*ÑUO?í³ð ËcÚ?´Ò4Lœ?A\æÜ3?Vcs(‰?²>BA›w?´»_Ò·‡?íçéiÂ;?´§¨òJ?"ýeҐ÷û?‡"%Ž$š?²±g@
°?–´·c͋?ïV©"¹(?mù><?UØÐ}?CoíÆj?›EBhºÒ?ÔNýš4FGL J1955.4+5132¿ì˜mŸA¤@'šoÅåÀ9†¸UFƒrÀ;ó€`°@m"M¥$g@çç†w~?¹Hw"^?¿†Ñ™»(@²¬ûv-"@õäÇ|¿ã¸×í'?2¿âüÕ©¿å›À¿èý,)Bï¿é'ìKî¿ïÿÿ&¦³AGNfsrqOV 591?ïáõ[ÉR?€ñÏ
Ž›]?N˜pÝ£º?dƒÖ(lök?gJÇÿDõ?x½X¼?ï'\~þ[!?—Ÿ_+?LB"'n¤'?^E/^ÑG?‰ä·BM?ŽEܵK[D?î·Z¬
C?ŠvjN¹?oc‹–?u;eÊ
Ÿã? œsTíé%?…Œdv‹{?ïGjOy?SË]yã?keµHü§?X%'°†W?"¯y<ñ=?}=µü xÊ4FGL J1955.7+0214?¢tÌÝH-À*l´¿ÍhÀ:D÷m5ŽÀ<$@µÒµD@!F0¿:'ù?üïçžà*x?À«˜Ÿž–Y?·A©ÿ©&?ü\6@'¥LUC(¿Ù=ªðÙòO?ïû¨LºÃ¶¿Ð"yA4}¶¿âñÃA2Ð7¿ØßÁœ"[¿ØqMJ5®AGNbll3FGL J1955.9+0212NVSS J195547+021514?î4FÑ/¬?ŸxçÂuº?x)Ä i?wd§,?©¶ZkyQ%?ý²ÁV¨­?îb,COe?­
Ú܆•·?w7»Îp¸?ˆr»vVÊ?¦ë"ӏàj?ªyqNðû~?ìM–݇ôÓ?Ÿ@A-´|?Š[½8ï±?z…GYzm~?ºC]œ;u?mþú|¬?çpôÕÚö§?¤Èb™Cp7? nÑ_±Kl?Žæçö¦]1?Î xP§Ò?¥lMû¹4FGL J1956.1+0234?Ø"Í:ì÷ À*EóFí$À:Æ3\MÞ°À<8x{;à@ O¥ï?ÿÂÑ¡GãÄ?Ñd£Ã"ô?ÖW»þžV@FÚhµÌ@ó¹Qoß6¿ë7¯ß/j?ïõŠ@`B`?ߺl¢ë|æ¿Ø8ÝâHßî¿è¯¯…")¿áçÀÃÿõAGNbcu3FGL J1955.9+02122MASS J19562808+0234250?í=å']ÒB?©ØÕÆÉÄ?'ùžh$?¢îÛñ`ˆ?±'ŠÓà?¥T(MÓï?î×f‡÷q?£³«˜í?peC^´?{¸zìzø? |õX1?¡ã4 ½¾?ê‡TôcÇç?¦ÿ›ú(Òp?£Ԅ÷tó?'ñ:ŽT;a?Áw
3)?£ž &Y?ë£JðáÓÑ?¡‡Q2–ü?•X4Íw­?ˆo¸E$?½¦k¾?¡™a¶V4FGL J1957.1-3231¿ß	áVÀ;7¼ä!}(À9üŒí¹¬À<? §?u@r⪯–†@–äÛ·K[?ºò¿¥œÝ?€{ ñbê?À—Á'R)n@	œp›ôgÆ¿ê b‹l¿Éy&‡~9¿ê$º"¦¿æÀ!ß&¡¿Ýsb"^úŒ¿ïçH®ÅzÉAGNfsrq3FGL J1957.0-3234PKS 1953-325?ïÌqãÞ?tyk/ü¥?Aʁ€í*?<ÿÁfÒ.?w¾öëËs?s¤þøÑh?ïºÕQ:Ÿ;?"#Øéã?(:٦ܹ?;RÙ¤fp ?€éÀJ¼¾|?"UðgßÂ=?îÞ¨¥Æñ?'©Ã`?|׃*¬ag?síª?jF?¤g%N¡?Žß/#þ?ïŸÇE}«?nþ"ÛJ?I$6Yqô{?9lnÝ$:É?†{ëXÉv'?m©\P¾Ó4FGL J1958.0-3845¿všªJGËÀ<öÄç%>À8P®{¨îÀ;«Ãæg@·RO@kÉÂbæ?£jåØÛ,?ÆÈ"D"š@"Ñ»IÊG@e:ÂHº¿Ït"çÙ´¿Ü¶}Àu%œ¿ä‹ÿG¶¿æ´Ka'bE¿ìO°â‹zó¿ê$Ɔ"ÄAGNfsrq3FGL J1958.0-3847PKS 1954-388?í_†¦Kt?¬®-¹U?¢a'¤î2??¡\ÍãLRN?§¦öZŒ¸?¡ýÆTŒÓ?íÙÙÑ[ã?µ"Á•Š¤ù?gVŽ<(?£ñ,_Î
?ª:gÌ-º?¯Ø¯§_?éôªW\?²B1áØ	?ºSëu§|?¦	‰cèÇ?¶ZÁÏw?«ñLõî¦'?í¦)ûòÕ?œa€SÆ<?—…®Ý|u?‰:›_ìZ©?©ÚÕicð¬?"Ê"¤§ÒK4FGL J1958.1+2438?ëŒEâÒ•À8*»À9Â¥Ξ^À;î*ëf@!,çƒ1xH@[GA1M?»1±×(¿x}xü–'?¿Ñm_BÊo?û¢ÝŠµ%;¿ï'Yԇ¬1?ïÿ…¡•ž¿ÊÑÖâOj÷¿äWF¾*rš¿åŠ ½zIr¿ù[1e8ûAGNbcu3FGL J1958.1+2436NVSS J195800+243802?âëÕë.|Ã?Ä`;@¹v´?w¤{î?vÌ1÷Ñ	¤?ÙÉßÛ6?ÄMe"ˆî?ÙÊC3Ml?Êç#âÉ ?z¯öø"DÅ?òÐ>{?ã=ºðvÁ?ÊàÅ6(?ڌ~]¸'é?³ü÷Oñ;?§¸Š¥<ZŸ?øwZ0Jd?á>8&Ïñb?²ôsüœé?âÒ#wó?±&Õ»¦å£?©{ËʋÉ?™Ä]½Ù¦?×;*xG¾¢?°Â¥¦wXo4FGL J1958.1-0711¿ëÍeàžT®À2Œ?>À:¼áÑ@ÏÔÀ<SbI¡3Â@ +Ôíˇ@_…Q
8Î?Ç{×ómK?¨.ÀÃæ/†?㍷ä{õ@۟@!®&¿ã—ëy`>.¿è3¬jVµï¿ã†Å~ð¡¿Ó:Êi²K¿ãkùM^X¿à½ÛÍñûAGNbcu3FGL J1957.9-0712NVSS J195801-071348?ïoò\Åxy?¬^¶éû-?;p`íØ?0x$XMQæ?'"ò%Í<t?¬^)‡—"?ïC{À,?'Ƙ hž?5 +dˆÇ?H†ÓiZïœ?Œ-ȄФ?'›™—z:?îªyoÆÙ?Š¯iÏÜ6[?b±FÿRÏÄ?M÷«ÜLMY?¤-Tžnex?ŠfûÆ?î0|¢}d?ˆ¿(:€È?QD)Æ?A°)IT†?¦¢Öç§`Õ?ˆa˜ç"èª4FGL J1958.3-3010¿¢%õº°)NÀ:È-œñ<ïÀ95íKÈUoÀ;Ùý2Æ&@ àZX?ý&ú@£^?¯ ö° Ï?˜ð|C6Oa?ì¿ÓÀí@
íœûù¶?ïïíJ.¿äÞv]Tní¿àR0N|e¿ÒžnÀ}¿ßœdпÕb¿¤(AGNbll3FGL J1958.2-30111RXS J195815.6-301119?ïÝÝыá?cÚAu1ƒ?+
ÂUń? ÜðzZ–?p8ÆÓüÉÄ?cO<ØϾ-?ZÝ7çq?€?
»\?0ùȞX7?EŒøÂXeW?€I€KÁ0Õ?$ný
?îǹimÇ?Šßˆ"Ÿ?hŒ@ncéH?]c~nǬ7?¢ b'å?‰ÐSû/?"Ä?†.zÉ¥©Z?cJ¦Öj"?Owb¶/<??£¡ev†Y2?…‰Â¾õXí4FGL J1959.0+3844?â@ȂÃÇÉ@%/<-­¸À9Ëx²Õ«À;'š0˜N@@q€»QO@1^aµ&¾?·¾Þ!³Ú?ÓUÃW@Ü
²p*@>3U—â	¿ÛW4ó&Ô¿äL#ú±¦¿çT¥ÿX:¿äô1•¤A"¿ïàñ4ˆs¿ïÿù³>†AGNbcu3FGL J1958.6+3844LQAC 299+038?ëÕ0d6n?´æéúRƚ?"×1–¤âq?$K*Ó?¼`°z5ö?³Ïv¦Ñ~H?äîœöì?Èéq°~«‡?¡=Õ
Vü?©Éˆ04,B?Óü"Ð}?DžV"›M?䎋â¡Â#?¯ÃBå£X"?¶! ó ?œ/å""§?ÑZ€ò"´?«]NחkR?ç5pol4?©›'{Z—?¤òP="v4?€ôͧ¹?Íìö.á1§?¨û¦¿à!U4FGL J1959.1-4247?àZÿ™ÂxÀ>ÚQÎÀ9]X «À<ä«ã£@÷8 ؽœ@(V£zÃë?µPNÅ_ñ?ŹH
°³@
Ár%·@ÆÈo(¿µVçÃH>³¿ÜMÍ=`Ó¿åªåò7Àa¿åÖmàXDæ¿ïS_²¿ïù7Y2¡=AGNfsrq3FGL J1959.1-4245PMN J1959-4246?ïu¹õªh»?­nªÃ§÷Á?tHåËKd$?€ ¹‰jÉ?ˆm¯ÀÞ?¬MüãiՆ?ïÎë°lHÉ?{Ÿ†Ž*Ì@?*´	Gâ+??¯øÚÂÄ}?w´‡œŠ6?{ÚC>́?îK"Ÿzàþ?"ÖùA;µ¢?'Ï_^Û»?‡¨g«!?¡ßH¢'*?‰$¢ì!e?ïìö¤Ün?OÓé‡K?.µ"q?"Ibƒ»`u?b°*ÒÚz?NpÒ¥ÅÄ4FGL J1959.7-4725?ïîÆÁ½F"À>Ø},{‰
À9!´:.Ï÷À;¿"(fQ@S±uƒdÏ?ù{üä?®Õ¼þ ?ÀqW†#Æ@À­Ù©@ö"Åš)¿Û¾P§ET?ñ³6#¿ÔÊ¿ÁÌh¤¿Ðï»dD£¿ß†—D¿ã|}`þÈAGNbll3FGL J1959.8-47251RXS J195945.8-472531?îiiQD®[?¡îÁ²›ßK?"#5Ðrum?"ÕLmwí6?ž¯ ÷¿O?˜¤l²Gú˜?ìÓúã?»Z1ÄÊx?›€1êˆñ™?«/ÏF¹š?²€"¼f«Q?²ç1è€m¼?æ¬ñà´Â?°<ø ö"?¸FA?ÅÕ?¢Œ4‡DY?ÉJ–gÝJ?ª"‰áN~?èÈå…Bà?¯yëÕ4a?¦A"©žoâ?"kE9&óZ?ÇO/ƒXˆ?¯*Qû(4FGL J2000.0+4214¿á.ÇÌÿ#@ÉéÍ³}À:-ÏZsÀ;¨ÕÑXLÈ@îd¥q>@]_V§­?Ãà™~욿 ]æ»?ÜŠ]ÜT@eLÚÏ¿ä×MÄ®ñ¿çûÃà•®¿èKÈö~vþ¿ä-RòK¿æ‹È ˜;v¿ïC¬ýúlAGNbcu3FGL J2000.1+4212MG4 J195957+4213?îq´}êQº?§Fw|`ó?QSOö!?I®yæŽ`v?¨Z¤Û3ß?§%jƒµ??í쬣ÍØ?²XãËZìÇ?D÷íu)?[9®Àņ?°p«¬æ@?²Ai»;ÓS?ë@H½W([?£…«¨')ã?ŒÑôõè?y©Ù˜Êz?Á1½»DÞ?¢Hä W8ê?îâjÌ?…ðÕ…>??Ï?©Ù¹º?2Y~Áb§?¡Ÿ±`5ŸÏ?…Z¯aåøÜ4FGL J2000.0+6508¿êŒ:
'Ö@1ªDØw$ûÀ6ï.¾YlƒÀ:é">¿@¸L]{±&?ü.ˆ>''ü?mJ—do?›°]ÓùE@Ô>š4@*æ';Ù?È˜=V«¿Ó¬%Ã'í¿ÚÄLÉÝ.¿Ùt-݈ݿà¯ÁÏÖ¿Ó_\òI^AGNbll3FGL J2000.0+65091ES 1959+650?ï¿vE»[?7f
Ã?Q"D*[A³?Œ¯Ïœ62?{àå}?xpÜ"½[?ï©ûpÔ*?Š»u'Èt1?WUØ'G79?wéÍ(
4B?'ÎÆâ¼?‡PŹ¥ó»?íCD» =?£ªàÚÔ¾?€}ö¡)Û4?|î
Ûéó?³ÖNÕÚ³?¢C§<3"â?ïóuÉý?Q"¾«r£ñ?±™ëe–>ýþm"Ëa??Yo‡œª£?QfωXO34FGL J2000.3-2930?çILWÏþÀ:þó¡LìBÀ9x>£©½ÔÀ;ýû›ût@>Kw1@‡ª4ò?²+g¯fµ?ªž,a™`?ôYè'u¹?øh5Uø/&¿ÙíÚ£úñx¿áf½+-«¿æª°þ:-"¿æ|ZYê
¿èþ»ýq°G¿Þ	5]ÚѝAGNfsrq3FGL J2000.4-2926PMN J2000-2931?é}¢­Q¶?ºû8ñ•œO?§ÝَÏ?"]è	ÙËÛ?Çôy¦àgQ?ºo1ñ­?ê˜gSÔ1r?¾¸¥Ð<ª?«ÌdoÔØÝ?²¥'r´#?½V")t?´1f.?Œz?é+4Hé?«GÜLÒY·?¤¸zNªR€?'Jºoß&[?Æ¡Ô¿"G¼?§J •DôÔ?鞲"þr¼?¨¢˜Û±ýÁ?µàZÆnÓS? yÈãý‹…?½*!–Ï?Ÿ{!$4FGL J2000.6-1328¿ïÿeÙ§ÀÀ5QÇ5ï¦À9Ãí~<QÀ;ý}K…9@ø‡Ô3@ÝS¨Á?·»júŸÃÕ?µ=ä7
?ùš£Ÿ¬Ù@ózÜÀ
¿Õ·"ÁÄO¿à®È4·—±¿è (ÿӊV¿èÓ}æOU¿Üöÿ<
È¿è<ýâC'AGNfsrqTXS 1957-135?ïl®íF¾?Ž_ò]?`x¦Æ'áj?q>³"?[
"¦Ì0?‹Y&ë^Ì?ïSüÁ¾@?"ÙM)?ZSyzDù?zŸ™$ ™?"Û00"§5?'R†–ûé?î|·«€??"/ó£'è?u¿±«"i?jó²J5Ƶ?¥|-2‰‹?'^ÑJLs?îM8®2øT?‹Lé®XDo?u êh?d5´²Šðñ?¨xr</½'?‰£´ób¨«4FGL J2000.9-1748?۞QêƒlÀ7çF˖lÀ8®Í"]"À;˶…ì>@Äm/ƒPW@
4†ðIª?¤®ª¢ÖY>?½[¦Õþ`?÷jÈ˶LX@P¨dÅ?ïÁcâþ¿àØÙ`ð¿åú%Ëk£½¿á4&­é²·¿èy4j¤9¿Öð-¤þ҃AGNfsrq3FGL J2001.0-1750PKS 1958-179?ïàxÄCºß?dðÜ_Œ?3¬ÚÈÝ?+ÿ±êé$e?m¸àì'?ck¢.£ËÓ?ïÑíÊGüÜ?~#Ž [+?59ñ4Ç?R8T—!ó\?u·w<îEW?{´`'HÏ?îûÉS:Û&?†m[uŒ­i?oJòÆ9¶?^Φi'?œw?Ýd‹?…ªëâä?ïÀ†±X?h$@,ð?ZÅ9ŸçÁö?KºWám"0?yXë÷‰R?e,'mlÅv4FGL J2001.2+4353¿ë—ô™Ö'ƒ@t3ÿ
zÀ8É16Ù±À;7ì]‹ÌQ@‹7Ö[û?üùä"rÁ?¢¼'Ÿ<ø?¸ÄP@N¡@«â´•žb@"7Ð%¿Ýù7Ēk¨¿ÚRðÛö¿Ö2ü´›þ¿Û!ŠßlŒ›¿â¸oG¶¿áö˜ã'4pAGNbll3FGL J2001.1+4352MG4 J200112+4352?°Õ€ ?"°%øæ&S?G;!-‡Ø?O
ðjˆ?!a·Ç‡?"Ə™bA?ï)­Z`ZÃ?¦˟Mw{?JÙ¢ÝD}¦?fOØßæÆ?™ó‡
ƒÏ?¥Ö½@0=5?íÉQ⮲?òÂäè{?ˆ‡$<çò?ƒå<!Œj?­IÅå¬Þ?šÖI'YÞ
?ïËÆv…,Î?hß4¤ø?ÈÁ>lÄZ?`<†ž¿?yµ¡¸oæ?hn:Ú~ö4FGL J2001.5-0818¿×i~–*p¹À3TFù¹"âÀ:Ш·CΌÀ<B
Ìsá@žŸä@OÒ}浬?Ä2"ý[
¿™f`ݐ?ىVá
K˜@Àû*XC8?äzfކ]¨¿å®‰J–ý¿ä{Ëóˆù8¿âÀ_C‡i¿Øyx;ûÙ«¿Ûƒ½D³«AGNbcuPMN J2001-0820?ï-sِû?È"JÉbÓ?RYäš=:1?\ÑZ²Œ½?™+æ"<Ëz?>föç?ï{Þzö{¢?¤#cš?BPeڒò?Q¥	U*+?ãWln>?ŽÐèB¼8-?îzÒYÃè?Ž×3£ÌaÛ?g'"Có?^@w+­?¦Ý?‰V?iÕ¹ÅKè?ÅX?…}Θ¾¼Q?JÆÐ=ÄÏ¥?>Zp›?¦"É'³kv?…~Î'ò4FGL J2001.7+7040¿íûœyP€@3õXÙµé[À:Ÿð˯–À<Mҍ.#@ùX…Ó8@ó:G#«?¸F	¤™|é?¯ãʝÑc?öGŬGH@.çÉþ;?×¼ÙûŸa¿È
‰*‹™Ò¿á7'Ô'½¿âa‡"à¿á`žü/¿çŒ:€¯gâAGNbll3FGL J2001.8+7041TXS 2001+705?îÙµR"?''	l$?n€ò²©Hâ?a‡®fýOf? ‡?I€IT?'1gj˜^5?ï?F:/«2?Ö@ƒ]õè?`ôæ"kg?kºRr‡îS?•ø›èLd?Ž¥aT0'
?îGÁÌ?'sW2Lç?|"=d¬)È?pž"]Ž?§ôoGMºž?ü ¦Ý¯œ?í77À—?_[2ý¤V?"G3!'Ó?wzœÄžç?±4u2â½?a77‡!¨4FGL J2001.9-5737?ê-/|ߎÀ?÷ë[-M@À:‹¹ÝÀ<Œà«¦âW@ðDK3…?ÿÙGÏ¢j#?Á·vÙ%K?¶W´ü?öB;C¢ìÿ?ñ>¹Ôw'?ïùPMö-¿Ô]Oö¸Y¿åP
nîË$¿×[l7`¿]¿Ûû+ÚÏCõ¿ïÿÿÊPËAGNbcu1RXS J200205.7-573644?ï»ã#@'À?|á#¹8õE?NŒ¾He?Fb¢iœ;?~LœÍÿW.?{ÍBÅÛ(?í`D¹@‹1?¯mQõ6Òk?Š\0·RÒ	?"fõ¬If?±²TLA?ª{NÕz?íìc 8Ì	?0˜µò?µ}ˆˆ…?s°ë[ö,?­W—LÂ.K?‹Üž0ë?é‰Ð–€p?¤'c4Ðé?®ha?ÌÝ?—y@"õ?Â>¥V©K?¡.ƒûþÐÇ4FGL J2002.4-7119¿ï"Té'À?@®û*®)À:Ë«®o´À<'°P$Ü@!ªñ§L‹?ùèäZˆ?Äþ2J€ì?¼"Ôeh±?÷r¦É¢@#'+f5?ïÿÁìžú,¿îÆŽÜ&?ÞSÇÝúœ"¿È1q'"[¿Üƈåí/C¿ÏpÜÔ+çAGNbcuSUMSS J200227-711940?î÷'3Ô?š;-µÖ?Dð©B¨
w?C,°"I"¾? 3'¸Â?š+
pë?îì–tI#†?™ß•=ª'ò?WÆ{æöÝ°?d´W–û£u? xdÜ6Ÿ?˜Î	?í1´o³'?™÷M™›Â?nµÿØ#
?WM&ãÐp?µ|¬Ž‹¢[?™ÅpöÁ?Ê?ì<Ћʲ? 08;…?mÿD ±˜|?aóòÔ|,Ê?½/_Vœ¬? ó–®ó4FGL J2002.6+6302¿×"öÃp@0q€²BÀ;qPþU0À<Ô®¥šXÜ@""¸;›6¨?÷¤G¨5=Ï?Ðg¼'c?ÐWˆ
€@=Óºý—p?÷ÙÙò$J¿í4DÀ¤Jx¿ïÿê o·?ð¿Ç—…BI¦'¿ÛåœFó¿ozFm!ÁAGNbll3FGL J2002.7+63031RXS J200245.4+630226?îì^[«ö‰?žÌyì6ùh?Wì
@®J?U'E`1÷ÿ? z¹Û@Z?žqT/§"
?ìP‡QìŒ?¼ª$•M"®?ŠiSOÞ?–Ck!híŸ?º.y¦Ÿá?»<ptñYþ?ìqt!Ä©?¢†?Ñ-?ŠCAƒøÇo?J$Äã½Ë?¼¬.rÁÉ? ý9<…‰4?ç#i».5 ?±	^×4u'?‰…KíÐ?†ê©/ú?Ðí1"+Ú?±4Ù'¼û4FGL J2005.1+7003¿æ+`Ío@3oÚè'®À9ðhÒQqÀ<#ñLÞÕä@ z¾©HŽ9?ú;o&ÿHJ?ºÀˌ°Ó?Å®6Jü@ÍÀ:S@ð6¿ãXò?Mé¿ÃþFïƒÜ¿ÑÂQž®+w¿Ð:² {¿ßGC…:è¿ä¢ Æ´…AGNbll3FGL J2004.8+70031RXS J200504.0+700445?ïÝvýˆd˜?cÞ2­ÑŽ?`OՅ³Y?UŒ8="G¿?b9ù¢´?YBóvä?ï–LLú4Ü?Œ|è(rjS?Qb'.¨?bŠ­¥Ùj8?ˆ@§à¬ô>?Š|
'Æ]P?îÓ¢ÔȪï?‰DM­?€Ê•ˆaDe?yÞ	=8Üu?&Z¢¹ÿô?ƒQ®?¼ü?í©npЋ§?Œp$"S Ð?s_ÓèÅÛl?_Ÿ¸&F€Ã?±~:ïE?‹"Áå©wÓ4FGL J2005.2-1822?Ô#šyðÃÀ8Gà·õ¥À:YEnŸÀ<o㽪@´"¢lQ@ÜòB9`?À¡âhjx?0°[@+kÇú*(¿ÛŸ¯È°š¿çèµ`Ÿ}¿ê@bUµ"¿â
r_C¿îØð²È?çý/Á
ÑÐAGNfsrqPKS 2002-185?ï5¾‹±?ŠŒ§¡ßµ?aÅõS¬‰i?_NhAÀ/?ˆA;{qñT?ˆpGUÏ?ïŠ6pu‰Ï?83º6#¿?=Ÿ)Yk?P/OR*ü0?Œ…j™¬™0?Œý»í?î`ëò2wï?"+wÃ0¥?~‹ÃŸUKF?w´b⪙?¦Èhí׋?'¢ÈÇeV¸?ïX³gž?ƒ",ú#ù¬?\:­ì¾ÌÄ?OaÈ>ÉïS?'>Á|?ƒ(ßáX/4FGL J2005.5+7752¿ëÛ¿*2Œ@6»½¯ljÀ8cSÒåë'À;ºåaïa@>®ïl4@"]ªÖ?œãàBSX?ª[<D\"@
ßE™›@¿ž$DÙ¿ÅN	¸»rÝ¿à'úáˆÁ¿ã¼Lßx÷¿á{¸<òϖ¿æÄÕA»a@¿åA".ÎI¥AGNbll3FGL J2005.2+7752S5 2007+77?ïÐ œé\?m$÷'÷ì?=lÔ¦ƒ8w?1&´3ˆ5?vä¦#¬?lƒ7©'u?ï¤.q……?'ž'³(Ýz?Kêäöz7m?]ñÜî}*I?…5µOV»˜?Mr8ÂO'?ï1±"Oe?'Õ© †wÖ?swQGDÈ?iOÂbÓ}R?"þõ†DB(?'®¿Ž'Ó?ïä­üÑùË?W´œ±Æ¬?;žÿ¸;?-lH‡¶šÊ?gÞ?jæ<¢?VhSü?4FGL J2005.8+6424¿ï8L
Zíž@0Å:æ…ÛwÀ:f™5ƋjÀ<7w^@1a¼­ž@†ö¼Š_j?Á%x	¦ó?ÏWá&öå@b[T‹@Ձ†R?ïòJ¶Ýw¿ÌÞXeqÉÇ¿åêûVM¯¿ãG¦¢–˜]¿ëÔ@ßn:¿ïùö€û=#AGNfsrq87GB 200541.3+641601?íÜ+ñþ8í?§@¡Yã?¨fö©ÀjŠ?¢5qv*^?"¬"l¸
g?'ìvOՒ?î'ô䓱??¤Áª _:'?{K;Pö?°zf´?£gJL¦+¸?¢"­x\¶?ëK]ë)x1?¨F'ŠxÞ¬?°Â2œI_ª?j"Mq'w?´âÞ
jÞÍ?œud€$?ëÀäi'if?¡ûBb#`e?¡ÉV¨ˆj?Ž}堈¬ú?¹Npœ?Ÿ~ž$Éw4FGL J2005.9-2309?ïžØE%ùåÀ:#'ˆÀ9 Á¶UaÀ;Þ{ÍÖ¸@HñS¿Å¨@19ÓÀÝ?¯XËH=[€?¹"IV
N@<êy…ýÛ@b¥ç…µ·¿ÕÅqú_r¿á.›‰]â3¿æô÷ŽAvÿçÌ.¬­¿æm¸¸ÇÝ¿ïÿülòAGNfsrq3FGL J2006.0-2311TXS 2002-233?ïú•o,|?=ÒÝsî~?$ý§.E?svpK?CI>®Zî0?<–,‰án?ïÙK¢¼Ä©?v°µ
X-t?$¤¢ÀÃ?@
Õwqä¨?r¶1|ŒýÙ?v"ÓW?ï-ž»si?~+»=î?nj™i†A?Y¸¤ í¸?–~Ù¤aü?{ÂZï\ù'?ïó9ÐçuØ?FEï#´u? Öz€àd?šC,^ ?WqŽàøAA?ER&@Þ*4FGL J2007.2-1433¿íê›÷³"À79~ºñ6À:TÌ4 ˜ýÀ<'¬-ðÔ@åÅj­É@¦rÅð9¹?̍ÒfÛ)?è% }ä\`@lûï¯P?ûœNOnRC¿à
sáÏw¿Ýe~_–~¿æÁ³"¢Ú¿ï¹û8ðâ¿ËÁßeUÅ¿ïÿþBe«+AGNbcuNVSS J200711-143205?כ5F³–œ?ÈsHªÜ9?ßÿvÄe?Êoñ±Ûa?Àʧêz–?¸ã³ËéÇ?֜ϔþð™?ÑÓèøt?ߍ¡¡ZŠÞ?Óà¯F/ž?ë"M	?¾C HÕ·ê?×(§®.?²î8±º…i?Ø;øuÓFÆ?³ºC¼Ì?Мã?«R[6íIê?»1Âìµéú?ª›ÍK¼¦?à°dlŽÀG?ƞà=_¹?×ÒÆkµó?à í¼ß/ò4FGL J2007.2+6607?Ó]H¥¶2'@1s›fù3]À9Ò"ÿ‰;À;ñgº#|Ý@¢
¢Ed¹@]e¼{a?¿2ŸÝoK?÷9½ï§@'¬'\f@lÐ"l¼l?²2³=ځ¿çòêmDŽ¿èÖÁ½Ð»¿è7çÍÚ¿ð?ïÿþR€ÖTAGNfsrq3FGL J2007.3+6605TXS 2007+659?ïÎ*Økâ÷?p&zàaM~?muéŒ$?gW¸5…·ß?dS±«}@?\®ó?ïF¥¹iª?˜Õ2G?fb{–§7Ð?y
ÚÖT?"^ù_õØY?•ñq˜¨"¤?îMüŸ$ve?">B?ŒDÓaç?'ÊF>"?¤/Øô&?‹fÛå_¢Ï?îó¹± ?‡$6ل'È?vñ#Š?e"r	Ê?›åší"¹x?…Afc<ÃK4FGL J2007.3-7728¿êhSjOÀ>†yF<û3À:k‹dL°³À<G¥«ö"p@.ß/ûÆ@F5~g?ÄxH:	ç?×±0@KA¿½ð'@¨žÑç¾Á?ï¿5¾§¿Ù€_ víó¿âûH
ZÍ¿èÙéëÁ"š¿ïþâßâÍ?¯aT¿Ü	½AGNbcu3FGL J2007.7-7728PKS 2000-776?î!w€Þ¾?¥AU#}•»?îΘ
¤Ä?ŠÇœ¼êy?¥q ¦±¿?¡'èñ?À?îhŒ—TJ?«çØÑ&£‰?w]À
¹`?ŠØiŒPML?¦‹~†S‹}?¨JJQKق?æ,·gáç?¯Óéjי·?Ãf-x6¤s?§%ââ˜è??ÃæôëeÓí?£èrÙ4j–?î>UKÛ5??ºL­ÒŸ?{YœÄ‡r?jº–(÷ß?¨¯w©É;?"C~«#X4FGL J2007.9-4432¿í´Eñ•ÐÀ?ؖþ´¦eÀ9tÓäCÀ<€§ZL}@k›@½Òtw?³–Ç'5#ù?ÀÖ­ _@%çñ@ccK©Ì˜¿Ù/-••¿ã™*]÷'¿çèÎUcä¿ë¼[ed¿æŠX^©¿ïÿÉC«P{AGNnlsy13FGL J2007.8-4429PKS 2004-447?ï恛'˜?ðYå¿ø?A´Y—È!U?kÔë±dS/?eNuâ?‡Ôk¦Âž?ïŽøoÙî?'Ë/Öê??Sî§X@?WêhÆhîÈ?‹GD"I¾?'Ÿ²üÔ?ïmÊAHÚ?"eñ†þy?páär·û?eïS8¶º£?š9͛(åü?ƒ"H'å?ï³ö•û^Ø?iÂ8?SªÂAs?C]aí«±e?€Ÿ¥(àV?ga#¼¨4FGL J2009.4-4849?·ú5'…XÀ@M!…Æ~À8.C~ÚÑrÀ;g1Ԏb.@pÁñÒk?ûü݆Xt5?ŸÌØؖ&?¤"^$Bú@é%»{k±@(ýâPm?×¹ø^ËèK¿Ö€A#5å¿ÚÑMD×J¿Øj¦sG¿á·zö@c¿Ð‡á@!X?AGNBLL3FGL J2009.3-4849PKS 2005-489?ïáº%?fîyæ|?#*	©ÉcÔ?öá0‡T?mÂ\«>Xi?fœ.ó
¸­?ï¿­Ø÷›6?€ q%yèÈ?1ó6fþÊ?G/‹Y?	àє7?~ý`³A?ë?'KÇý–W"?tÔîýÞÚ¡?q4±é!1Ò?£Hsð?¾XQrï_?￸"#'—?nŠò‰ñO?0'ÝÏÔü?".2™dp?#4Àa·?nO´?O£
4FGL J2009.9+3544¿æTáž'W?õÀ—Ì:À9«ð©JèÀ;8&1Âð«@ 'ã'ØD@‰éÍ³}?ÑBDþ·«}?ºëÖÂæ˜?ëȆ·>Æ@	eˆšî®?ïÜyGêz]?䪯k"¿æäMÝX‹1¿Ûì{ÿ)ì8¿çgš®lu¿ãÙÎ"7bmAGNbcuB2 2008+35?áω‹Ò/?ŝÍÞQÅ?Vd¿	˜—?S¤[ÏnÛ#?ÜJˆ)R!O?Ś«…ðº9?à$D¾Å?ÍY±!‹?êDA?—~ùâC'B?ßpþæ$r?ÍE"áñ e?ãé1"Óö×?±WË*´àL?šÇWÄ-?…¦}~&ª?ց,"æf?°´sʃî?áÎWŒÔ—»?°Hkæ¸A?Š(QPµ%?|\òùù?ےÌJà?¯ç3xç'4FGL J2010.0+0726?Êß9¦®šÀ+}|o½'=À:"ãY×À;Ô¨ÒÁ'@7ŽÆÞ@M˜¤§Ö?ѓ Ì"Â?Ì5¾=gêu?ùZÔG'‡@Ë-´™$T¿ïÿH è?ïòøp¶L¿æðf…p¿é$©'¬¿ïÿëþ@bF?ä"Ä?µwœAGNfsrqTXS 2007+073?î¯"¹ïBI?Ÿíš•r?WXòÈù-?€8£éTí? ·þ$YE?œŸë2˜å?ícNu"	ƒ?²Ä@øÚNÎ?'cl?RÃmób?°Œ±3-²Ÿ?­wKV¦]%?æ¸?áXÝ©?¬tódÔB?°=v5^R?–q‡¥ÙW%?ÍE`Ú4?¨ÍsŠ–+?èœ	_½ û?«*^ìa%? tgHt½C?ŽMOnïs?ÉrÀ®ìLÄ?ª'ÊLx^4FGL J2010.0+7229?¾',Zz@4*Öý¨6ëÀ8Ö§i¦À;пB Ž€@œÞ¬ôd@•ƒb¯É?¥f¦R9³«?º‡[>7Å@Ñ2^!‡@Oø0Ó²o¿Ã¶¨@οâƾ?ì)4¿ã<î
ö¿ä'õÉEY¿ç£S¿šµ¿ìcÝ ÁAGNbll3FGL J2010.3+72284C +72.28?ïo+ãØ.?¢*$0'ež?l}íLøü?‰#Ý]XÁ?4ç¿v¶c?˜£ÛŒ%aý?ïcLˤ…?—má dtI?p•ú3j!Ä?{®þ–!»?™nÙ°æê?"`/Žç?îÝfÅ?'D'¼Ki?‡1i¶b$Þ?…óyͽ†?˜Ãþd6JÆ?‰¸F~{*p?îcˆU¶?†ïȐ?Ž	#¶Rÿ?sLaÍúsI?¢Kΐõäî?'ÓEø½±4FGL J2011.6-1546¿Ûî²PÛËÔÀ8°0ã͚RÀ:vJßø#À;Ю2­Ò@ûÒBØl¾@–ž<–‰?΅ ¨×z%?Õkã=|D@²fŸqIï@é^‹P«"?ìÓÀ§$œ—¿æ"Ÿè¿é­Á±ç¿íŒQGpÅ¿ïÿñò÷¿àšÓá*ÕAGNfsrqPKS 2008-159?ïl¬AM[?"½@-K°?ƒ•Š?Gþ?ƒlŠÝÐ?ÃZ1-a*?Ší;ˆƒ¡?ê3ÓéƒLŒ?¿s†_	
%?²ªš^çã?¶Væ1×Ï?¼Y¶†³Â?±¢|x}÷?é,*#¶?«°ò}är<?¬ƒØîBÂ?"W3idÐt?Ä-ð×Q?¦Õ"±fA™?å1`ïè?¤¦ùUùî?µbŽtÞõ?–ë™1'd³?ÎÙónÐé?£§Sëǝ4FGL J2012.0+4629?éÅ.Ê\žÖ@sò«´NÀ7ùvjNRÀ;+ü™C3@щ³¢?þÌÀmBùz?¡ð}^®Ø?¹DŸÂ'­C@±þë-@°fŒQ®?î~Ó-A¿ÙI‰`çK~¿Ý%=ð%—¿ÝæúÀ¥÷÷¿å2Hø"¿â!Ý Y§AGNbll3FGL J2012.0+46297C 2010+4619?ïyÍ ?ƒäL?éFÉ?NáÃnœÒ?KTæCâ‰?Îð‰­¹?ƒ8Þës?îMãcõÂE?²ÀPÀÕD?a}¢°ހ?ª<¤?ª	ÝÔ?²vÚ¼Ù?íšÕ\§¥?^F¶eY?Šp&"Þ[?'36'š¾'?¯Ã©	-Ž#?™Úbο†i?ïTZ†a?"øÔS?X-"ÑkŽ0?JùÔKG!?"ñäâ$è?€Â°WQ…%4FGL J2012.2-1646?Þ¦çô#0À96½ÂmÎ:À9‹¨"ÉX¤À;DŽŒÂÂ@ê¾¥AÃ@¯ï¤h)µ?¼Ì8A(Ù?Øàc¢¼­ñ@³}pn'@	˜JA¿Ç¡QHòã¿ágºú<q ¿éÖæ+B¤¿ìKâV¡Í¿ïÿs+(x¿ï`,Æ1¨AGNbll3FGL J2012.1-1643PMN J2012-1646?í­ú+&l?®Ân›Ü\‡?±mÁx|–[?­¬Ú»ƒL¦?r&Ò÷£dÏ?u4FKeï?ênoiuéF?ÄÇu'²?µÉ±]{'
?¿oØ;´É?¶ÂÓVÕ#Å?²ì'þÏ´R?åŠp6NÌ?²ìê9È?ÌØ&që°?°˜Ã<Væ?¹ü2*¬
E?¢G'8^'?è{é0?«q«™o?º®ÉÝ÷ã?£c¯œ)ë?À¼7›CÅ?¤è‹Ä³é4FGL J2013.0-3717¿åÇF½Ý#À?‹UX!)EÀ:…Þ\AIvÀ<OÄøÂôÝ@'T-©±@ØIёX?Å6>5è?·æ4|ßN°?ï/_¿_@%;Qå¥â?ï÷5¡L–\¿à—¿9fS¿åÜ=ƒMÕ¿çUr¼Å¿è
g'E?$¿ïüÁr%·AGNbcuAT20G J201248-371941?íÖyURäÒ?¦•ÀI™u?gôøÞ¡ô8?_2<`–æ?°ŒŽsɾ?¦fçfÑæ?îkÜðñm?§"Fu9CG?d}t^­PÞ?p ˜–'‰?§úYªþZ4?§u"M•B?íKFåՈU?˜¶	x͌"?…ç"9½µ%?sŸ¾th?²è䊯?•ã9ÑÄÝ?íc]êν?­w$±'?…_÷âŒÆz?m½[š»?²9­8~a?‹2
ØXŒ€4FGL J2014.3-0047¿ÙíXð©mDÀ2¿õÆÁÀ9ñÎWçG¢À<l­¨DW@ >eû²hs?ÿ\ÝP¨?¹›ý¢È?™µ ü"?ãcÓCßRá@
±ÇP·?ﶿ¹Sž¿á¦Ç…ò¿à7@=ݱ!¿Ú1Å{`¿æmP›#•¿Ô'xŸ£ô¼AGNbll3FGL J2014.3-0047PMN J2014-0047?ïÝ°»½‰?aq8}ÃF?6؟$¦"˜?)Y79›Tå?otÙ_­²§?`´m&j?撚#u¦?"¶×ԍ¬n?4Ÿ]ÝAE?BÞEaM™?…¶¼3Ͼ?"Ö5™z?ïǜn}<?šXãËI?f¨3r1ç?[À7|¾nX?›²â[?€¢ÈÖý‡?î)aàþÍ?ˆ¼RVuå?r(w&ã3è?Z;Յªä
?«$à­¬Â?ˆ
Áwp4FGL J2014.5+0648?͘xUëÞ¥À.ï»À:
†¢F†À<MÝÙd‹@!/òù²3?üæÑáÃô?¼"À^ÕMz?¥~ü¤¿?íÀSí"?üÑPÒÖQ0?äÔÀ¡›EÁ?|jâ"pv¿ÕN\¤›«B¿Û'oü'7P¿Ø<EÀÿd$¿Ü‡5^0·ÙAGNbll3FGL J2014.5+0648NVSS J201431+064849?í>îbÇ?§]8ç(_?r>má¿H?eàºØÚ4?´ç)®ÞÝÐ?¦ÀHJ¿ç
?s®?¡r¬÷°,÷?pÆ?Š!²)?|DŽ‹ŽÑ?¡õV#"Žá? ´
'ËÏ?ìF¥yÑà¢? 9%IÜl5?ˆ¯nE?w¸YüU?ºÇC¯N?žhÒi·?çØuÉr«?¡Pc¨UF?ŒŸ¾9·²?"úb•!¡?ÌîJ1þ^?¡ËȽUi4FGL J2015.0+1621?æS¿J¶»À$L'ÿK¥À:{gkÀ<™%ÖS^@7Ã¥†·À@!Ì{n5h?·?äq"&Á¿˜Ýèº$dÊ?ã K.Ò{b@5O&óû?ïÿíöé	¿ænyÖ]¿åjŸb0w¿ågÕÒ/]¿Þڌ}ý0Š7{í6OAGNbcu3FGL J2014.9+16234C +16.67?èîmÐ8?ÀB›*Dá?ÄÕGq{|?w¯lÝÚ°f?Ë)þ@H"j?¿Ð"žÌø›?è`
Ëéöô?Å`­z¹+}?c-q(Q?t×J"?Î3l'¯?Å8»¾Äk'?é­õ˜þ²?¦¡E½8dÔ?—­Ô›™Š?"àå7?ÆRo.(Óö?¤Á)oÄ?ìß+xž?'Jý`oë1?ƒ'ÜãhÚ?o{ep3"Á?¶—K bµû?'ÑÔeò4FGL J2015.2-0137¿ìWQ
õÈ*À3T?Ä;-ÓÀ9+O&®ÀrÀ;¹Z%æC–@ۙC]x@™ä"rÁ?­'w-|?¹;#ÿŒ@}ÔÇm{@êñ#?ïý´'l¤¿Ù妢ì~™¿ãgwÞ]îÉ¿ä§''kþ¿ãå{ð;fÞ¿ìY!¼AGNbll3FGL J2015.2-0138PKS 2012-017?éÕº–?¹)Ó+Tµ?"É£¬kßY?'*süy?Æ/À '™?·¥'¸%Z?èOn8œº:?Ãøø™œÁ?¿‰r	âv?ÁV7'R?½û17¸#?³ûúWŒ´?æöcÝ¿l´?±µÐ¶â9?«ÓÕ2E߂?":Ɨ%Ä:?Í1{<pÕL?®Ì÷
œçç?áÒÄæ‹~¨?¥ÞF(ôϝ?½"Ù¼´?¥¸¡'@Ž?Ôõ³<yÕ«?¤7Ï9I4FGL J2015.3-1432¿ëèü¦.RyÀ9›Ø8;À;`þ{›ÑÀ<º­æX@!NoæÂÂ2?ÿÌbäѦP?Ë+¿ 'Å濖HáxÞì"?ÐÀ¢\‹Ç@
°s3©OÅ¿ïà¿]x?ïúkHMw¿åL8½¶¯¿ïÿþó…õ?ïÿü¿ÙŸC¿ïÿý`éNäAGNbll3FGL J2015.3-1431NVSS J201525-143202?ïý6<?Bԉ­ª.>ôgùUÆIw>ùs®œÈ€•?6Ìpñ¿ù?BuÕPŸ0ë?ïføTñ»?¤PÔ>j´o?IÇô)ŠÅ?kð‰]Ì!¼?'RµÍ¨|Y?£n:³Ýkè?íYÁjÐH?¡[0"‰Ð÷?uí·.u³­?|¶Í6eœã?³ÓÂ"†? Å×â"(?ï…ám~T?…®v¨qÖé?@‰NµD)?#J³Â#?Žld/õœ?…©Í­Ö—ã4FGL J2015.4+6556?áaù}Á-@0¤_¿ƒ8.À;tÿ†]À<%ü·v#s@t±ë@ËLÂPr?ßF¿¢AÞÈ?ái¥`!Rá@kÕÓ܌@ˀ"düY¿ïöµ™ª?ïd!È`¿æò
¿ ¼¹¿ê_ ®
ë¿è:´|lb¿ïþ†ܕ˜AGNfsrqS4 2015+65?í¼¼úHn?±VîÜ{ý?°óÙ\°¢?±.ܬR.?r¹‹¶°¾ð?q}?"ϪX?æ'_ß)؁?ÊÚ…&?Åè¯Q"®?Æ75Ÿ*…a?À
тL?¶¥u>™?êŗžÌH?¤Ï«ß±´?«ý–‰ë‹?—³Ëӝ<©?»ÔxN×û?›ÙðACH'?ä=ìN{>Y?·ìíç!¢Q?Á
±ŠÚñL?²ÂAqÒ[?Íú;8P?º
Ië'½4FGL J2015.5+3710?륛N¿D"?óFç_ö	ÝÀ7OE0‹¹À9¼°´hQù@ 5ä¾[@¤H)í?¦~qcß<U?ÆÀtå/D;@"vtÑc5@TÊH8(¿Ü	"(™&¿Þß9K{(•¿áˆ\ZséÝ¿æj>B(¿ë'"ÂÀ'¿ížè]RlAGNFSRQ3FGL J2015.6+3709MG2 J201534+3710?É	ÄÒjyò?Á£…ÇÅÐ?× ü ?Î^Úâü®?Üxõοç?ÏØõÂ|G«?ºÉÕÛð©?ǎ/ý‡í?Ö»Ðhue?ÔJüÚ¡?ឨÝG8?ÓýœÈÜØ7?Ó({Ì¥,?³øj]ߣ?ÏC값]?±•|Õ/S?Ý6+ê,U?¶˜šÍìÑ?Œ÷fÁð?|OÂIx,à?ÁX"¸Œˆ?µã†–5ü?ë66Øm?µý@»Ï‹§4FGL J2016.3-2331?éIˆ½±ÚaÀ<†·þ®ûÀ:Ò<!~|À<°¹ßŠ>³@˜¥àyÒÕ?ÿï¤h)µ?ÉÎu™_7?àc·_}>@N1ÿVŒÕ?û[(g¨/ß¿éò^VÍl/¿Ëº!úP¾‰¿Ð2!zÎþ*¿àY	†'¿îZµUů¿âþ@Bæ/AGNbcu1RXS J201604.8-233049?à$›¹~
?Äö÷ðÁ?Õ1€ZH?ʒ]wcc?Å
'±S<?¶¬Zò÷Œ?࿨Õ¥€?ɳ8®yz9?Ò¬¬8?È:Ð$&Vß?ÈÑ>sPùý?¸uÌàgô?Û
Äòº?¶Š8#[?Ø´ ¦Ò?¸Æð¸D–?Ȃ²¤4Ìå?ª7_'?ãs¶]³j«?®÷J­šðð?ÊC¡ñRò?«À[câk}?Ç턗à>a?¢L¼Ø74FGL J2016.3-0903¿ï`2j`qÀ6÷ƒ8.D·À96œò®3À;ÃÖPM'@²ÐG«<?ý¸¸É	É­?®ØŸ¾Ì®ð?µ«½ž¹þ@ŸIc÷ ]@+3¥Cò?ïó?Ýæzž¿ÚS°àˆ¿ÚsŸŸB%¿àáö?6÷Ž¿ÝåÌ¿çÀÞLQkAGNbll3FGL J2016.4-0905PMN J2016-0903?ï߄Í0n?fŎ*óê€?7›4ã7Cê?-þDKEgÔ?m‡ÌPh©ä?f-úªîœñ?ï'	%·Êà?Š>kV»Äg?GþôQWàS?_xrt}5?‰ýÇL÷Ê?ˆk:Ïî?îè=Ò¸'†?ˆ'9»•$?tcS™3•?oýîÝ)®ø?ßp ê>?†T½üø?í8†à78?˜4wÜA?rNƒ§Ûüµ?]'}²X€?µàÃÅÆp?—þ·Oۘ4FGL J2017.5-4113?Ã4֎'À@µA•Ì…À:'~Ù#óÀ<yÌí€@ Á-Ý2ö?þ¡™'ƒÒˆ?Á†~Ëb?¶æMý8ûI?ö¹Ö ‹%c@•èO	R?ïŒo_3l>?²Xúm¿Ú|²ÙÀ3¿àÎ1†ŠÉ¿ßÂLì¿äڅ‡"ݘAGNbcu3FGL J2017.6-4110SUMSS J201729-411516?ï ‹^!?yæ4}6#?L"­£Y%?>ÎÖQ'æ?Šõ»]‰´?y>¡ÓÁèi?ï[D6ÛôÁ?Œë¡MÙ¸?E¾;ä+¹?S8 :È[?"é‡E`
?Œ9Jd–?î°,]‰?"?ŠD'";Í{?nÑV"¹r˜?b¶&&eÀ¶?£$¿ p‰?ˆcàr¹=?îx a÷bˆ?"çtý:'?t\¤^³?`îú˜~ÐM?¥êwž5K©?"[_¼¼˜4FGL J2017.5-3753¿î?ï,¯F»À@E*"8…À;ñ¤óiðÀ<Ö)làÔ@VæÌzm?ý
v
HX?Ôá5"Ç$—?ыt¨H‰?ûLv›gÏó@E¼uÎ.¿Ú?%ðz|?ïïUÑ{¿ÖÝ~`X/l¿áвÀ12þ¿ßݜÞr'˜¿ïÿý¡UûŠAGNbllPKS 2014-380?ïܽ°y?jHf@i—?Aȵø2.¦?;9í¸Ð°Ã?nÐ"Ûo!?h™£ÍHºÞ?ïNÝׂÒ%?œ"8$݈?N1ˆúe*e?jKfª??•2¸ÇҒ)?™­¨K^p<?îH½§«Ã™?AímlM?'t§pśÍ?wû"úTì?¦Öû©_]?Œ:•¸Žè?îÛK¸¡ºì?ûZg/Cc?U=†+ ™1?IÝ;=ü™ô?¡¡XD‡La?™Qk!f4FGL J2018.5+3852?ÖÎNãÏ?ú¬løQÀ9zeEÔöÀ;Œ 4Rî@ ²þ¤‹:0?ý5¤ãc?À"úˆÇº>?Ò2¿-{@
}ܤ±$Ñ@󟳏%¿è.Ê榓¿éàz~¡Eµ¿½yG'R¿Îk~¾¡æÅ¿ãÊ^'Ӄ ¿ë–BAn	sAGNbcu3FGL J2018.5+3851TXS 2016+386?ÐÅtÙ™@?¿Í«Ò¼×!?¦Øã<î­? ™249n@?æ/·_¬ÈŽ?ÁÒä6?Å^»ðìLø?Ãޕü¨0?£«¡¹›}?²éNÁ†1"?ém–è+4ð?Ä:•úÊë?Ùí	œëû?²JedåN?ÃNÂoFö?¦ókî³?Ük•+qjô?²Ôµ%:ŒÈ?Ù9cž-ˆ(?®$‡z¡¿?¦´Qep\e?"…S_"Ó?áø	'6&?°A{'Žø‡4FGL J2021.9+0629?é¥ÃOÝÌÀ0Çñ"<:CÀ9Ô¦ló"À<›ûs©E@hþŸ'¼³?ÿ8B·4µ?ÁzØù«Ó?ÃW"üÑÍ=@uîþOý@s''dç?ïùd:<;ð¿ÜÔ¬ÀþZ¿Ú­.â@§e¿Ý•+uϐ¿ç6‡æ鮅¿æ䡟øXlAGNbll3FGL J2021.9+0630PMN J2021+0628?ï<òÐn
?¥Ü"ƒû?´~¯´B?¥xæ[?t†F~Q¯?"°
%?îÐf3J?žÞ(3¾Ÿ?s÷?;ñ¼o?}Ùz³Ð×Ä? €ñµP³Å?›eôëÐ?í§¨´³…Ù?™ªÈ'±¼.?ƒO7' ™$?x
…Bqœ?°XÓh/¾?–Ø
¿j÷?êØ£p½ÎÇ?—æâíà?ûŸ=O '?€?¸Äà™?ÀÝþU^àÖ?"ÏLPog™4FGL J2022.0-7224¿ÎëÀ|v7À@H6âëÀ;_~À<½~«Ê@!"˜`©G?ù§»/ìVÖ?Íҟ_+^©?ÊâÙih7?þǧÓï?ûðSå…U¿è"'|É?ïèw'î\j¿â
Lõ|¿Ä›Ï¿Ez³¿åY"‰ê¿ÄãA-qÓAGNbcu3FGL J2022.2-72201RXS J202204.8-722538?ïI[G(2?‹Ò ڃٚ?\ƒP
øÜW?`ï!L˜NÒ?•b¬?‹(z÷ñŠ¢?íáâìÇÓ?±ò¹"âeé?zÇag')?‰x)yj¬Ê?®ª¸å'}?°çÁ).4?íæEOñÕ?'«—2ƒ¦?|÷Õü­?pvøXh?­üÄ0^C?ð/֋lg?ë´×šÙ?ž\[‰½K?–½a.ÍKJ?†$¨UX®y?¼©êã•å"?œ»ÎÒw¸D4FGL J2022.3-4513¿ïéñJÛpÀA;—ædNÀ9•s³VBÀ<þ+êi–@±ß*óH·@+sKQ7*?°šï¯û°»?¹ü¨ ‰Ò@	1eәo¨@§@,ÀÓ?ïö+ÖGŸÒ¿ÔçÃK•U¿áÃ1­÷õp¿ãmOŽ³ŒŠ¿çätôž¢î¿×|0}d/AGNbll3FGL J2022.2-4515PMN J2022-4513?ï™ZÁlÓ?obvŸ&?FC	Ì=F?BŠ©)ïª?ˆIt_z?€ÙŒ*?ïy
úÇÀ7?&…Óz?F)y9j¿?Yò/ç&Í?-ï[>-á?Ž" ù®*?î£ÆÃgΘ?ŽjCæ{âü?|G‰à("?sw¸ÀÄx×?¢:¢_?Š•DiÏêÅ?ï{cqÂM?€¿]J·?d–?i`%?QZzÅôà÷?šˤ›±À?RïŽX»\4FGL J2022.5+7612¿éC¡Êˆ@5#1;â.^À8éÃ5tVÀ<²<'Î@ÇäX¯™‹@íòœj.r?¤Ò' ½ÿn?¡ñrsï¢?ùÿ¢È"§@oÃgp~?ïÏ"‡"‰¿àâ¢Â7G•¿ä»dàTi¿âA3¦ö¿åÍ·þßn¿åòGAGNbll3FGL J2022.5+7612S5 2023+760?ïÆ<î–çý?tí3{Ÿ?C<'¥ðS_?@ƒÏí2Έ?zyöÍ÷??sïºèa?ï•MGý±"?‹Ar0Áº?VN×UÎx?oTXÞÁŒ?‡âÓÙËÕ?ˆéXôßâ?ïððRØ?'ª´Bb4?n;ޛ¶?`»áôÁŒ™?˜Ïú•Ñ ?
'ÍP†"?S½Ù†?uà"]‡…?t5ë1{Œ?b‡¼9Á_¢?'6u…pàÕ?q
§ªt4FGL J2023.2+3153¿äþŸvcšÀÀ½gý?[`À9¡ §?tŠÀ;oÆÐ3‰š@!]´8×7	@qú[{PÙ?¾lðï÷ä?¤R×¾Bph?ênwÂYV^@lF__áè?Ö£e_Ö)m?ï±ß`£-í¿Ù¢'ÌM¡¿âç!A™'"¿Û؜cÎ[˜¿á‹ºžLèAGNbcu3FGL J2023.2+31544C +31.56?؈½ICë?À«ol/ñ‡?ƒ«Á(…Ë?zž¬Tݖ?ãlòV»óJ?ÀƓ";MX?Öº@¥é.^?ÄÖ¢ŒÒ?núx¸àh?~db,ª?äƒå¥'¯ï?ÄÕ±_ÈÕÖ?ÝM¥\Ȫ«?´`¿*ÖC?¤™)ÞÊÜÛ?‹¾ÅaŒÿ‹?àš³®üÜ?³¥ò3{?à9^Èù3Þ?¯_5ÈNԌ?¢¢ªùQžê?ß
#"£¡?Ý8íãdg?°´Å¯f¼4FGL J2023.4+4127¿çò}ú	y"@Õü¦¯+ÒÀ8ÿÊñ*z'À:ÕKoj'@ wýFKê@Œ~»ÇÁË?Áõ…Rº·÷?Ä·Xtû@B"~ea@wóòUk¿ïÿôa¼2¡?ïÿ
ÂPÇï¿×£aÔÜ;¿â(orŒ¿èќªÆÈ¿Ý#®ÆQˆ‰AGNbcu3FGL J2023.5+4126SSTSL2 J202336.19+412527.0?Â?úÅOÕ1?¶M >y®;?ºjé@!›?ºÀ…lIŠ=?è"¤&©€?Ãr£|Ö¢?Í,	nXs©?"ù7Îx‹?¾]7ìÞa?ÁvTò5ä§?äéZlGJ?Æú¥}&Ë¡?Ð-eze§-?°ùÜën}?»8Ã+
?¤ýgs–?ä'4ÝkŠ†?±"F@¯VÎ?Çg²þå²Ó?¥Üøýµâò?°4VÔ%¢?"©õÓ¡µ?èˆeÁðw?§ÿ+gšµ64FGL J2023.6-1139?×vSʾÛÀ9­Ð¦v ïÀ9Y´Ñ-"žÀ;õSì^ó@w#Ñ@yî?ÿc<Ù¥"?¯·Úø3­×?À­aw"6-@ã9:´0õ@
w헝•þ?ïÿ¦n£¿½eøØCx{¿â<XuâÛ¿à¹_²˜¿åë'H'@	¿í'¦ïnAGNfsrq3FGL J2023.6-1139PMN J2023-1140?ïûÀ]É?"M&PÚ0?fxGb?`u¯úîëA?‰úqÖñI?'Zõá|´ú?îЋü†Íy? ðd"Tu€?tÙ®ëfÛ?~VՇ§GF? \ µ»?žXتx?îq¶éä?žuOÄB¤ª?—M&œ´§?')ÿëRå?¤BQCj÷X?'¹…ÇV˜ÿ?ìÇr*ýì?"Ú"Àl?™ÞŒUœ?¶¾/Nó?³7(üû:?«\šJ@4FGL J2023.6-0123?É]ȒÖ[íÀ5þ÷ÂDÀ:[§ŠóäÀ<U›ÍP€K@ÁË[ˆ'ß@Íp`»?ÂeãØ×ó?ם 6×,¢@ÏÄ~I±û@ù(uj?ïöŸ>I;Þ¿ÓG>'òŽ¿Þh3Æ)ñ¿â¡ÎAÒ¿î@;#Â|è¿ÕS"g*±"AGNbcuPMN J2023-0123?Ê&|0(=»?º=ù©D*?àXæÍ<?Å{·ÂI ?Ò<•¶F«?À-7§Öë
?åðK4x‹¥?Å,NçNº?ÆtÅu>"ì?Ã,gÚáG?ÁÊ
¸ß®~?³vŽ«|ÑÈ?Í¥?;[Áž?µ¸›Ê6žš?áåu5Ñ%ê?º´‡¤gÞW?ÊÄëí_¦º?ªÉ·m0»?ä·Ï`z]S?£6p0±Ìf?Á•ÎǦxú?Ÿœø´p?ˊó¶p¹?œÁ& R*4FGL J2023.8-4828?åã?!uhÀAz»˜Çâ'À;L-ê
ËÀ<°ìˆ3@@CÁNêHß?ÿû©Y*=Á?ÑØ
¢gÉ?±ÉòQì†Ñ?Úµò€:¢é?ÿ·	Øi
?ê0‰jwm¿ï5§¡ïÿW?ÝÊ3)ø÷οÜĄ¿Aô¿ïþÍ?äF'?ïõ@‰]tAGNbllPMN J2023-4826?ï¿lÓ¨ç?xãOäh
s?ILYèöɬ?Gó™7ôÁ?} sY³´?w¯È
gö?ïBYî?™¾l@î;7?V´ã/QF?f'%[Ù¥Ç?œQ	ŒÛìö?˜mÑvPse?í迱²d÷?'Õ\\ã?†,¬üœ™?4KÁK3?«èÙäZ‰K?Œ(Ø?ØèY?î½k¨þYp?Z¡hø@£?`+ža©×?Z^VTJ+?£&‹Ng?ŒÅðyïޞ4FGL J2024.4-0847¿áŽUÌBíÀ8¥"¦óõ0À9Ë,´"ðãÀ<#:Š?‰ƒ@ £Y5ü?ÿ!{zÊ¡y?¹×Ó2Ó?ªñÆ+rõk?ñˆڀ·@ùyŠ˜?íbfâ(r¿Ùuã'¥¿âg…_ÐË	¿Ü%l 9±R¿Ü
EbàŸè¿è©rÀü¨AGNbll3FGL J2024.4-08481RXS J202428.9-084810?îåÉåï€m?â‰½_fê?e×ãbêF°?Wò'ܹ­·? EãjÙTÒ?¯½ÒÞ?ï6YŸŸ+P?"JñÌv°?Vèj[f±?b8—:+
U?—ÆEfd*Ý?'׍àO?íûœ¹h?™"ªÞ«?"¯f¥Ú¶?tC£)ŽÅp?´¢B
`C?—7ÐWw>~?ìUef´Þœ?•
"¥ÄBË?‹
ߝƒ¨r?sw_5"ô?¹óxÖ¨–?"ô;M+4FGL J2024.6-3252¿ï™=´À@rö@c^À9[ù‹q¸ªÀ<YhQ"2@'ÝžVAÖ@хÞz?²#Š•š±?Ã}ƒa@êÿÓ>×@¸	™¿Ø¢PA¶Ù›¿ß	Û !³"¿çqž]£Ÿ,¿æªõwÖ¿é¼]°	s¿ïÿ³©æ÷AGNfsrq3FGL J2024.4-3254PKS 2021-330?ï´4ÅüŠ?¢e>©ë?a‰ê"Õ ?yQªoÛ?} §¸lÏð?Ÿ@dÏ'ò?ïŠr( ¸?šIù¤?CÅ÷»ÐOð?WmýÐi?Œ'|šÍ?Þ¨BeI?îÿŠÑ`)?"|Óô§q?x—õvNa½?n^IZ9±?™è°è@bk?€Øôhç/1?ï‡2ۏ†?rÿñ•EA?c5e×Ç×?Q"àR]Þ?‰r;¨ˆÃ?p—j:ܞì4FGL J2024.7-2328?Á'¨MðŒÀ>Rk?éúÛÀ:¿ìMøÀ<€¾‰¬½@o¯YIre?ÿ3-Ú-Þ`?ÉõDæf?ʬ¬è*÷@&ûëýê@ÓÊJ¼?ëM¾,0
?ï]ËB83¿â›6A°y…¿ÜÊ®DK‰k¿å5¯¿ ¿S¿ïÿý¡UûŠAGNbcu3FGL J2024.8-2331NVSS J202442-232826?ï•Óáñǟ?€.ÈM8ú?j£BåתÍ?mÇQlQ´?ƒâ6Ê-†?x³¸L(b?îþ(v±åš?œVŠ€¯Á?bðÂw‰y?nê‡pÖ»?ÜØÚÒ(é?š¸+éc´Ð?îIâ´?!wjM"?|•)ŽWµñ?oß^z™îõ?ªÈɝæÝý?‹F®ûR±¤?í1?̀
?•ÇTÖ±ÍD?–,kžÀ?ƒR'äf¿?°ñ{þ¬O¥?'L3"ƒ+4FGL J2024.8-6459¿ßLòšo`ÀA'žÓ•>À:ˆ¨½ùË3À<†\S½í6@%ÄRTá"@(\ÅÓ´?¼øӐá9@?£cV9?äÄ°¾Ï3/@ÅÛAÖ?ïý@h¿Ûšðü××m¿é6ù5¿ã‡!A™'"¿ãmÝô<}_¿éMOõ^fAGNbcuPMN J2024-6458?﹌@³»f?€ÊèÊe6Ù??CþÞÙ/?<™soŽ?€¤í³/è?€;TäüçÓ?ï¹XÄè9?'TBpQ>?%@ÖÔ7y?<y[ÜQ]¿?TËj©"À?ã
\>-m?ï'fNt?ƒEœÇ'Ï?lƒÁ'»y?`{Çd¶N?š}e"òZ0?'Ž×
*[?ïÓ¦ŽhÊÿ?\ÐAŸr›?AU~F‹ež?0¸5ñ{?t	ɉ?\õÚþ"44FGL J2025.2+0317¿ïúýÏÏ
ÀÀ3`4óþÀ9:yÂc½?À<®Bž
B@gÑØÐ;A@†ÛPô?®h¼ày/Ÿ?³‹ÉLd²‡@çÖs>»ý@«é¯¼'¿ÜFï}¦ÉÙ¿ßða<æ¿ã«DAM}6¿ß¥Iû÷‡¶¿çnÅ°xÙ¿èç(bõ˜žAGNfsrqPKS 2022+031?ïðbøFµî?k!q!âg?-‹'Æ;?<@«"'¹?[ˆª€›_7?gíú×¢d?ïÔ¤²ÖŒÄ?zí$MI¨ƒ?1h˜hx?PÒúÁ‰Å"?t—Ó-?x£;ÿ?ï
|^}?…Žúï?kì/qÐH­?^™-öíQ?›0Š†‡k?"‹1'f?ïžÁýZ^n?nöŽ¡7Œ?V)KÞòX?Bˆ"K2?…ŠW-Š Þ?lñXïôxÌ4FGL J2025.3-2231¿êBŒÜ5º;À>"ÓÍ$áÀ:‹Ú¨W¢À<nU•]ʶ@ '6Ö*ïm?ýégØVmË?À¦´_B°ª?±Ìö%‹«?óá3ÁÎl	?ù»fØ&G?ï÷ڂû¿ÜªWA…[t¿Ý¯ïüý—¿ÑÙ÷¢äF¿èíòKâV¢¿|>ûq-AGNbcuNVSS J202515-223016?î$
Þ~?¢¥edŠ±?nG)ŽA?ey4þ|}?«Ú¶ýoB?¢3"Óªâ¹?ìûZF@y?²yóB@"+?áÚ_à•Ï?•j´Ü¢§V?´hôYÑé…?¯<¸L@ÑF?íM"Û½X?•9ªÿë_?'áó°<m?wƒÇ¸?³;㇕?"Æ'ÁŽÉÚ?æ?ÝþwK²?¨>L¼'ÎÃ?¨Ð¦'¹T?'.V!õío?Ðf/0ÚH1?¨¢Tpe'˜4FGL J2025.3+3341¿ä•ÔZµ®"ÀR

ù¾À8A=e¼{À:™-BŠ¿@‡/›#1ˆ@Ò±-4±?²jî «†?ÆÖhA‡ß³@s ÔƖ@ÉÃØÝQ?ïÎxžwNì¿å«ã‰o€¿çý"såªê¿ç8?!(οï-ád´`¿Æƒ~_pAGNbll3FGL J2025.2+3340B2 2023+33?ì°4hu*?²fסkn;?§þ©gön?¥…9«\4b?¬þ·óì?©‰b&1Bß?Ü	±«¨/½?ÏúS'q6?ªèçz;=½?·n"+¸{R?àL˜²ˆ4E?ÏK¤f÷ Ž?âžø¥Oä?µlZ¡p‹	?À"Nr`Ë@?¦,°]©g?Òç|œú—?²ëdúž¼?օp×Ê/7?³ªˆ3˜•?µR*løî? È	6Øêf?âQIF?´@•³c74FGL J2025.6-0735?æ\©»ÈÀ8cY§TmÀ7"§&J¥À;;A¼bò>@t‹gÒ¢$@ƒÅ_AË?Žµë`ðR?¸ÝÊ @&sü"$íö@ Bî «†¿Ð7X[á¨&¿à9RÂÀp¿ä¸;æ`Ê¿åýÉÄڐ¿è½jęød¿ëS/uKAGNfsrq3FGL J2025.6-0736PKS 2023-07?ï¤,ÜNù?uØ=ô҄~?Rü>}bì?Qd.¿5l?"•Hdré?tVÈ5àÝË?ïuæVùÞì?"Q†…d™	?Xvî=*Ç?hכ¬7Qƒ?wŒyãÇ?'P¸—ò©?ï<蜐6#?‡Û2_™rð?…9_ïs³?'ÿ!Á¶¸?‹ÂŸ|ƒ?}I<ÐÍ?ïÔKÅëbè?jgÈÃÐöh?L"Š¾ƒpo?I‡ãG?rI‹²~Y?gÛ·qȶ4FGL J2026.0-2845¿Ö7ùÁw"À@"ƒ‡ß]À:˜i6$;À<Míض@HLó"Ìß@dqcðja?͘+ˆy?ŜÆʪ2Ä?ö–•ˆ'á@	Þ'h#ֿ湓¿ºëy¿âÇ`Ƥj¿èýب£!Ù¿è"u'À²¿è¼ÕÞÄF¿ïÿ½ÅGóAGNfsrq1FGL J2025.9-2852PMN J2025-2845?ï'"H'?Œè•	Ï¡Ô?^«/"Pÿ/?]Y'WÔ?‹¢Mã»?‹ ŽLŸ6?ï?_ÄjN?‹Y=¬?VR¡ÈÞ?nÞ	ƒ}\µ?›Ö>ÝV.N?›;çŒ|Þ&?îµ´"]Ñ?‰)ìŽ7Wñ?t¦3f ‡µ?gâz'Á?¢~Jöï?†yõ_,`¤?ï*X6)c*?~ÝyÃKNû?XSœø–ƒ?FB+¿p
v?™/¿y'?~!Èð`)4FGL J2026.1+7645¿ïü¸Tg,×@59>ê ›À;
æ_E	õÀ<«­	¸æf@"Š[Ö?'<?ø›%:L,(?ǝ¤ÖŽ—ˆ?ÆWe—‰t@‡ÿÞr¿@T=ïϱ¿ïëUN.K¿ï×ßàzԈ?ïå³vQì?Âv'^¿à´€€G¿¾³ÌÓ¯ëAGNbcu3FGL J2026.3+76442MASS J20263126+7644487?îpe@dǜ?Â:ïÃÜ8>?Ues\Ô½•?T¿J[ӑm?¨N€^Ìà_?Â?(<t|î?îäØTٝ‰? çà°4î?iâîªf?v%ÀB	´"? Zc…Ë?Ÿµ
êd'?í~ã
•þ?"ÃP:Yp?yŸä]Œ·ã?q0êDJI?²néd"Ž?"Äã¥
¥?ëò8½G¿?¤¾ûƱz?}/t¢ü˜?y˜º?¾œgw×R?¤9¬ÁÌBá4FGL J2026.6+3449?×͍™ÂE¿ÿu
xŽ‡À9¢ZÐ0.œÀ;?Ö§A"	@ s¹£¥60@CÂÍoŠ?Â8Éu)wÉ?£ùÉÁ:ف?âUKÚt?ý3ßJӸϿîÓAáKßÒ?îj»_¼þù¿è`¼mÙø.¿Þû]Ay¿ã–,A§j=¿ç¡®pÁ3<AGNbcuNVSS J202638+345022?×Taj.]?¿_rŠÌêa?‹¼y÷呀?‰fk µJû?äcçkR‹?À%Åý1?þ?Ó6ëêçD?ƑåCXš¡?}hõa¤àç?†"äv¼ ?æ)¸‰ÇBœ?Ƃ^¶Ùœˆ?ÓbÁzˆ³%?¯ìÂb<ò?«II'VFé?XäënÙ#?äš
©¦B?¯c^ϨP?ÚHÅ&ˆ×é?¬rŠ-GÆ?¨fœXí,?'è´Â»÷
?áU<ö8?­Gù¦M'4FGL J2029.1-1839?æ®Od¨\fÀ=£·•-#OÀ:°dPâp£À<kَ|/&@ˆ>	P
Ú@ÙaÃiv¼?Íe˜¶×í?Ó@ª; g@EQÄ?ÿc‡ÁÕÍÒ?ïßÓ™hF¿Õú,@ûÆ¿äTž›·¿åÿ`h¤
¿åU'ÿùJ¿ïÿqšw+AGNbcu1FGL J2029.0-1840NVSS J202900-183709?íEY'ŒÖf?©
nÜ$ä?‡fPúë??}rÉ}Âcè?²á‡!yïg?§À][†Ÿ™?ì4ʳL?±žRÄ:ù?•óªò£·?˜(Ó!õYî?¸Ü¿ªÔ±S?­}ˆO¹À?ê¬OÏs°?¦&2²
Vç?©uH‡'|?"AÔ¼?½ã`·L? E£R.œÍ?綤0Ÿ;?¢R×´i¹?­·Ê£Ãp??•ñ.œ?É·|—§?¡èÍð%›4FGL J2029.5+4925?†øMÿÉ@ª@]wúã`À9õ6À;jÍë°½£@´Øö¦ºê@×R9ˆ·Ê?¶ÌMöØäÞ?ÓA­§m˜@ÙgÊêt~@ó,ª-®?è$ÁUuR¿É/¥ßøù|¿áÓ+UïÞ¿èì›Sþ¿ëF–½FG¿ïø3þ_AAGNbll3FGL J2029.4+4923MG4 J202932+4925?åòùÖÉë?¾X°+9#?›"—xï?¸ÄÑâ/T?Řù,¤?µzíÏ]?ì	Â|Óc?¿°ÈÑbá]?~¤íV¢.?sP†
\?½ÇCúŅ?¾ö¢ú"õ9?ܓJb]'?²j¼mFM?לÿ.ðÑ?±.[çȐ»?Ȥ1ÜÝc:?«î)ùeq?êÂ÷BFv•?¥TMÅÆ\:?šnÁªq?†KuéÅ9?Á¦JÄâpa?£sô¬
ß4FGL J2030.2-0620?á{sâ-¹À8Ö®::ŽqÀ:GÖ(ôìÀ<%o•º@ǯïœZ"@qƜ1#Ž?º…࿝å.¿¨>,œ§QN?êG±ÚØÿ
@C×n;qñ?æ*K-$ü9¿à
è`ܺ¿é·<­/x"¿ÜÞ>ÄáÆÚ¿êˆe>É…¿Ä5»"ÖCÄAGNfsrq3FGL J2030.2-0622TXS 2027-065?ïÔ¦s	¬?rá{Ç»âm?Qb&œè­?JP
qǁ?qTuüÓð±?pÒEr-»U?ïÕ?ÊeCA?wŸ*šïM?%C n^Æ?A-§H6I?t´ ´Zì¶?v'>杨)?îûÜ-q¥D?†¿eAß
?p!¶1`¾?g$zÄÿ}8?œ|ÅsV?"zÄ_Ì.W?ïÌÔ¦k'?a#åRô–?:z"Â4?(ܖ›Ò€[?wôL–¡òÑ?`¤+dÛÓ4FGL J2030.4-0502¿åù*g¡iÀ8Lma,jÂÀ;,,"ÜÁ7À<ƒØÐç
Á@ ZÑÜV,²?ÿ•;fœ?Ñw'w?«)ˆ9ŸÞØ?áj‡þf¢Ì@'šËrړ¿Çӈé:x¿ìxþžÖð<¿áÿ®ÁžñG¿à
ïAkÛ¿Öµ»€Ê¿á·1$e:AGNfsrqTXS 2027-052?î©HžžR?—ùµ^´?FêW3úµ®?;Ö·Àºò?¥ÌÃ&/ý?—Ì9ÐeJ"?ï;˜«ØÌË?˜>QíÍ??QûµäøÇ÷?c£ðתD?—m/&–Ú0?—M%諸?íÐwzӛ(?'Ü3Ë^ºs?lFŽ÷xØA?[³ÅÆ?°š±§`
?'aÝOÄ?í÷"®Â¡[?kfY¬d?DðDŸ™€5?==Íá^Un?°'«Â!?§©$"4FGL J2030.5-1439?Ün(ýzÀ<o"}cÀ:¶Fà‡•À<yŒ†‹ŸÜ@ çþ¥aùÅ?ý©•?ÇR¡ãj?žŸyzÀ;?Øß#¦@@víb£æ?å•6Þcx¿è»îQ"ñ¿àÍ,¾¤ëݿׄH"S6^¿ÏU-Ä^iB¿ÕC¿ÝÑAGNfsrq3FGL J2030.5-1439NVSS J203028-143918?íłټ›B?¤Çº,LŸ?Z•Ð&\Bá?^²årDSû?±i'ñ´Ü?¤¡fhn=?ï\!s?'x½°m>?E1Žüð ?U¡——§·Ú?"ÂУñ^Æ?úZâàËh?íc'uÜ+ ?™/QuŠ?q*4y²ã?aO¨ûŽMÁ?³ÐÒí×Õ?˜|"$qš?î)Ϟ3<î?Š*!Ô=Zt?YÀ¦p7.o?O°Ú<úq«?¬•éJw³?Š%;f·"#4FGL J2030.8-6959¿ÑË2Id‰(À@ç]þ¸Ø#À;¨mqóbÀ<²˜§+R"@WR
é͏@ځNš?̧ jْ®?²ú2¡ì?äyºHeÊ@ßËZ'œ?íqD îÍ~¿ìKIt¾þ¿ÅCŽõü›ò¿ç.ðäJ7¿ÜEva†,Õ¿âg¡yâÅAGNbcuPKS 2024-701?î"Ä ϨO?™˜Æö¸–•?U2½‹»É?H†²°·?¦
(
Ù?™PÊ<)å?"Æ?šJ˜·#3¼?T¯ÆtÂc?e†_rÓ?œÄCa1ËH?™*>®Ã.n?íƼÜ»F?'¶á—O?z¸îÁiè‹?kõ5ƒ¨û?°‡I?cæMÍF?îçʸôDH?èÙ¼ìÞÚ?V‡©â®?I>"`h ? Ï'Ü¥ü?©	r4FGL J2030.9-1621¿îÌiÊÀ=0]¥qÀ:®p¦[HüÀ<~b¼ºh@]µ%ç@…	Œ³?ÅÛï?z?£ö AÏ?à_‰gó.`@œ¤MQ¿ì0Ï«¤¿Ú6à;êfç¿åyÄ6%¿×'@~b¿×.ž
œ µ¿ïÿ"Év7AGNbcuNVSS J203048-162224?ïdMËʵ?Š˜ò¸A?L¢&ù>3?A>´`	‹ä?''5Nòê?‰dPÜ?ê?ïSübÔË?˜oö¬®Ãä?A"ÆO%o?WÆdЋ'ô?•ÂA,>-?—®®ó]™Þ?íó™A	Îs?'z‰ÿÞ?v+M¸œmZ?bAnô`–?®8O‹?'`–)j¹?îªV°=éñ?‡ŠÜrõ&Q?]Ì[ÊC?P/:|î†?¤l4ÑHªš?‡.áäcû4FGL J2030.9+1935?êW•âbÀ'
"cØ­À9¢^)ÊÀ;î=ÚV"L@å4!Å£?úpŸM7Á?·›þ£´{?Ä,ÞÅÈ¡š@°iS@/ÅÇ
â¿Ù4åOz'—¿ÚF0ÑY#ˆ¿ÖCÆ=çl5¿Ï;>š@¿äŒÄŸâ¿Þ|Û·Ì5AGNbll3FGL J2031.0+1937RX J2030.8+1935?ï5á5È?"þÜåÌ0?€üÈLÿµ—?@ç/?Åu5Ç#?ö!Æ3?îð{q»B?¦"›uýÄ?a¿"*cò°?sj©ä?Ÿ¸ŸX|o?¥0©>3N#?íÿFß#Æ
?šR–SAd&?Ž÷¸?ˆ)ð	!•?¨‰Tµ?"$Ý"Ž?ì?ë™U0?œ"ÅçÂ/®?'
4óyn?k£¬À™Ú?»¿dÆ(Ä?œ*'
‡à4FGL J2031.1-2615?Úoh£Wˆ}À@G¦a(9À:‡îúôþDÀ<Â*²[1@ÀJˆdh@&†|†c?ÄZQDÁ%$?χ>.@bϾÔã?ù²jÉ!œˆ¿ïÿ"=ßßy?ïÿþ½à ¿¿Ü‹©_>¿çN(Ÿ~¶¿ãf[)òB¿äGGQÎ(íAGNbcuTXS 2028-264?î*4Ôè‹N?¨^"
ËG?‰»*#f?…Öœ¨L…*?¦íè0®…‹?¦¥àK'á¶?鞚×dçf?¿1†~ße~?­‡¹Èú?°4¸}­J>?Â"2³ú#å?¸g:^t{?ë& !@D'?¥)(¸l ë?¨ÍOÉóM/?—ÊTwh?ºhW4à?ù«6w?é@Ia_žþ?¥l<>0«U?´-É°¯=?Ÿ˜|'K?Àçõ¢)üè?>,x}T24FGL J2031.2-4121¿½øopƒÔ>ÀAÕ¥~ª*À;.¦Üx;À<³JÖ½ç@m·&tU@?e¦MC?ÎÖþÎ?à­]€ä–î@
¼{F@¿òRBm
¿îCšžý0Ã?ïÿÏù§÷*¿Ü/#" ¿æìÎÊÓοîCÐàWÄ¿ïÿ–ƒd£ïAGNbcuSUMSS J203056-411906?ëPÌØß÷?Í«J¬¹'?¹AlL°0í?Åú(ÃBÐ?¨pYØ -½?½ÝQI»,¶?ïI4á:­?›é¨Š¹"?]ò¯a¶p?xÃü
Õ?"ú8éCo?—Ø`ˆ¨"Í?è²)Ãq"Ä?«pKµ'?¾&dÜAC€?£µ€ç-?¼HM2[?žãu>|?ï‡K7ËðÅ?yÏQu£Eó?qA'?¨ˆ?cDxâzÕ ?…£ycú?w:?Օàº4FGL J2031.8+1619¿ï¶¥l`¦À+ÿŠ:›À:ºZ/ ~üÀ<?Ô|ñÃ@ó2Ûõ^¼@P³''d?É1Á¿"?½ä<Uäˆ?õ^yLò÷Ú@&¢¬ì?ïþÔI˜Ð¿å.)ÿ,ñP¿ìgß?–ÀÓD`,;¿í©¿Ãyè¿ïý›l°ÚAGNbcuMG1 J203139+1622?î½×"?¡FTh@¾š?ou¤	B"h?q>*ä?ž?¢+5G)æ	? €•×Ñ=?îÏW§Ý¿ù?¨A"&tPÊ?gRë{j5Ú?'ÿÁ— ?¡•VÊm]?§2¨4ËÔ}?íËՁ!?™ °UŠkÙ?ˆž%\me?{ëë'Oò?´ܨsɝ?—_×ÖM?íqE$Ϋ ?œ_aMÜϓ?Š¡Âü•y? ™"`ë?±!žy÷óÙ?š¦-Sž'z4FGL J2032.0+1219?íq2ãAŸÀ/"š8ûÊÀ9ÃÁc>ÓÀ;ä"Àìĺ@)*Û£@ž®"i›?ÀCŸ¼ô<¨?Àìõ·&È?þ]†Þ«òb@Ç
ÈÀx¬¿±	[]ô§Ý¿åcØ·¼šP¿åʆÁ¥§D¿äG-»úír¿æ¬L#Å&¿ðAGNbll3FGL J2031.8+1223PKS 2029+121?ïî+#ô‰?UŠÇ»Ê¾?@ßqÒyÚ?;Oë15¾?[eðÏ¯l?RÃX3î?ïµ½•™G)?"GF1¤}¶?<²Ç€¯Ì"?W<Ó/V.É?«]¨·}?'ñÝ­L`?îß~ŽC É?ŠW8ÁÍ?u.B¾C:?jº\>žà?žÄ¬æìUò?‡wÙ£ÍKÝ?îj Í×!«?‡Çr3™]?umß,žÏ?]
b}ý?¦¬Ef¨Qt?‡Jð<blê4FGL J2033.7+6308¿ç:ß²,¸@*øœýç!À;CÛ÷âûÀ<—έwœð@!'x´FÄ?ûÚ®‡ggî?Ì£J(î?Û@=²¾@ˑcj2¤@›KutK¿ïþ³™õßì¿í¯>;¤ò?ïÿÿ^ðP`¿§œÅ+	¿ßŽý'¬¿ì9Z'}rAGNbcu3FGL J2033.6+630987GB 203249.5+625814?í^µ$ûð?°ØK潔?‹?~jÚÂ?ˆÀ{?36l?±˜oO
Å?®'M¶Q+a?ë¦*mÉÔ?¾:Pùdèý?•v×ZM'?›S-Ø$?¾¥Gö»ô?»ÆS"áw?éŽq¥¹…?©`ÔçT±?«'y¾#u?˜K˜ûKôC?ÂáÝè?¤lœ=å?ç¼Ðqê?²§¼Yåøc? æŽq/	-?šòu<:?ÌÓI앴?±ïΕ€†š4FGL J2034.6+1154?íS_ތè±À0Œ¬¯öÓ1À9YiÂ;ySÀ;Žpð›@r¨h3@ÔdcP?½-—ÿÜÅ?Á¶—;?þi¾Å£à@k–JYÀf?ä"ÝÛ
¿ÝÆG·J/¿ægfÁ€Š¿èFl*˅¥¿è'áý¶z¿æXøŠ.ÃAGNfsrq3FGL J2034.3+1155TXS 2032+117?嶺'èý?€ˆ·\}'?[ÛC2}"?Zrˆu¨#á?'ñbŸpó?}dœ`#?ÿ‹5l?‰?ZÝîkæ?Hgž—N?`E*c'ƀ?…‹O#I/ý?‡t–ä3b?íZòÊPfž?žá9ó²µ?'Î¥wrk?v aÚ$;?²Î"þŽ}§?œ7"Ø©¡?í©²ª@?K—P‡¥?'ßMÝãó'?iWt•™Â?°W(®ò‡?ƒ9CD"C4FGL J2034.8-4200?á« Ml3ÀB3´ÃÁ‹PÀ:C¿šµ"ŒÀ<a,"¹º@ W$"2LX?üsAü#Òm?Á¬ÐB£¿?ÁŒ÷Ÿ´:Û@ô즆çæ@db̨å'?ïþ6Ò$$¢¿ä杞6€¿ß¿YFÃ2ð¿ÎxÕäÎv¿â'jeÏg²¿äìf€<¦OAGNbll3FGL J2034.6-42022MASS J20345108-4200386?ï½4©Q2À?t¦'8›ÿ?G•™i ê?BïüÁK­.?~rø*CÝ?sdž']>D?ïL6ûèów?'æ;Œr?H7¡b·?Q÷šÜvé?•·cwËØÝ?'› X«½Ô?îãž?ý&?_ù÷@C?kBåÝî/?[	±ÓÎx³?¥pQí¢N"?ŽŒ¶E†çþ?íì±t?ˆëw\÷ø?yØÊ`–Œ?cʱ8]ù?­ùÕ¬¬»7?ˆ4žò¬ó?4FGL J2034.9-0450¿ï㷊p[ÞÀ91öº «À:tBúP"–À<N¿ïn¸D@T¢Ëò\S@b¥Z'"?Æ!Ô¦Šî±?Âþl©±?úÆqÔX²I@Mq6Ô¨¿êá:­z÷î?ïö'÷䨌¿äSÓâ?Ð¥¿äÈ'­ÄÊ¿ãÏ >ŽÛû¿ïø²<'ÎAGNbcuNVSS J203508-045029?ï:úHrdÞ?#"Šû?l× òh˜?m€üãü!e?•ÂÓfa{?ŠZõZ'?ï"-?š'GÊBݶ?_Ùëü€Íi?u0˜)qíù?šîÀ­¦MŽ?—‹Kæ$?í!dF4æ6?™É&:Ä?‰|(‡^?uÂëšÆô?³ÑnIGÞ!?–ôÊ׫4?í¸%q¸áð?é¾ÔâË?‡cÒ@v.I?s¢¡‹?®¤´TTU{?Š¡k8!f4FGL J2035.4+1056?ڊQP\ôÀ1>F{åS¬À7²¼MùˆÀ;4Oó]Z@zø?kQ@".:¥î<?—³®e%0?¿¦Û ¢ŒÝ@"'o°'@}4JµZë¿Ë kÅËÑ¥¿â%¦V]Û¿å<Z#bØ¿æ£Pg  ‰¿ê$¯â±;¿èæÖcNƒòAGNfsrq3FGL J2035.3+1055PKS 2032+107?ïm$ÜL8?€¾à­;?{?nÅuî¡ß?g¼ê"åo?1WvUÄ?}'æ?ïª×rƒN?'ÿ-ðº¨?Tªe§ªl'?u8ïͶ'?'´Öª70Ë?Q¤UØÁ•?ïú»{?!KŒfÄ?‡x¯<ŸÙ?"µVýߌM?"ÄfŠA1?†ô>»_q'?ïÃíƬã?qc"tÛœ?Hq,ÿt¢?@ÄKõž¶h?zú÷q	 ^?pѺi
R4FGL J2035.9+4901?ӝ¾ÂH@ë@UZ¥À9‹'ªhô¶À;¸‹C•@ Ɋ8þyB?þŒÜò´½â?¼eáÜ(Šc?¼ØüŸ½?þ‰Às"6Œ@­¸ºÇË¿ïòö—¡qÕ?ïýŠuV¿âé>›A:¿ÒXÚaµÒŠ¿ã€¡{k¿Û‹ÃîúAGNbcu3FGL J2035.8+49022MASS J20355146+4901490?íàmíB·?°YƎÂÜ$?vÒaâ-Q½?«è'ô3àk?¯#¼äæ*d?£íýFõÊ?éÕ«¿<?ÁEåöW?y§Þd
C?…~ˆXÚü"?Êïjc¹â¦?Á&>·;¹?鋬eQ¼?¨õÎã"8à?"t¸¬gÎð?߃×+$?Çb·U.ó1?¦÷*JéžU?éßQKGý_?³Ôä£"v?¡:9å§þ?ˆ,Ī®>†?Ä4,Yv
ÿ?›ë¿§ie4FGL J2036.4+6553?ï¾¾Qè]«@-—µÐ1\À9ûžs.À<(Ød°ƒÁ@㬁u`?þº}>ïÿØ?¶_adsòì?ÃÅ£e@	Ê*[]@
,™­æƒ?ïþ;¤ñ¼p¿ÌcÂÈ&C¿Öë÷öFC¿Úå»d°¿çÃâB׿äLD琝rAGNbll3FGL J2036.4+655187GB 203539.4+654245?ïßnm¶'®?g›úŒÓÑù?KF¥>?EÌùÂY¥?iÉÀÅoÊ?e¡OâB"?îÿzm¢?¢p²F N?eäÁ¤Ô®j?tói1/ÓP?T#¨6?¡¤Ã3Ù³x?îß˺Ð`}?†úÙ<3¡?ywÍ4ˆpr?s ÌMÓ?¨•XÑԃ?'ìØ,ö™&?í*ªÈ]Ë ?'UmÕêQ?–ý ?ô?{>ŽvÐ]q?±'ju©þ?á…øÌÍ4FGL J2036.9-3329¿ïxÁ†-è,ÀAśý÷èÀ:^x]ï"À<H™¤T(@!$/_>)?óŒïœÛmz?Ð.è¶7_?ÏÏ{¨Â×V?û'ÿ·@¨éÜ?Ž¨ºH棹¿è)!ACAH¿äLXÓÖ¬J¿ÃÃ7Îxt¿Ê/ÁŽ«)¿Ú&èa¨¼wAGNbll3FGL J2036.6-33251RXS J203650.9-332817?êÊ¿x%?¸Vá¨-Ï?{ª/3¨æ?uêð8‹?Ãþó°D'$?·´s.ç·?íÄQE?©5sð=?Zù%…®Hþ?pk	‰žÓ?£°÷yh?¨Äù°é5?êJ
\ÖrÌ?¨zÅÚ
W,?—5ì渐O?ŠC×‰«m?ÃñïÏ"È?¥(J#̎?ê¶×<Ž%?§‡_Âÿ3Q?UŠÏ8E?R1XS±â?ÄùoWfÍ?§{Exw4&4FGL J2037.9-0504¿ïéÙÊ®†ÞÀ9ñD»ó¡À:ý]0\¿À<‹;Óåj@ J@–H+?ûGã>(Y»?Ô2本ž"?Ìÿ9[–S¿?ûTâæÅ°?ý?]Rìa?ãc	¼Ad¿ëI‡î'ð¿Ï1~¨&¥¿Ü&š¢þ¿Óôk0Ñ¿ïü>àŸ°AGNbcuPMN J2037-0508?î
ù̆t?  Ü»wc"?fpI%'«?`¨k
ûb¦?¦ˆÑõ?š? 7,ÀáÜÅ?î\rz?IG?¥°(ØW:?oêO*ÃÀ?xÉRfýÅv?¨<·¿i?¤fÂmü&‹?íR·^öàÖ?–ç_¥oY?Ãw't<?r܈­þ~¨?³1ÖúxÓ?•'èp=uõ?é_Ðà¡n?£L™F,#?t=ˆ"Ôî?j'ñ4?Êä"x][¡?£€Ï«nÍ4FGL J2038.7+5117?å"`þú
@ÿA<á1ßÀ9g{o'VÀ;A_ˆü"d@¦ºZ•@Ó}c-Ø?ÀúX R…ß?Ó±Zÿ@¾6`]'@ˆ"ŽJ[¿â°¿?ñ\¤¿Ûò–Šñ`*¿äÀ~«Ê*¿èÝ_ìú•¿î¿ñQçSa¿ïÿW-ä>ÙAGNfsrq3FGL J2038.8+51133C 418?èâ¯lT#R?½}aˆ3Ì?¡•@ïW+k?žçºx½?ÈòÙ§Þ?»¢x¶µó ?ì;Õ('Å?¼axo ?u'аù?^Ñ9ˆ´ª?¼*ó¼Ì
?»i`A?áõ–tœÑÚ?°¹ú֑?Â…- +L?¥±~ü¼ë?ӐöF§?ªæºþÓ¥n?èöêçÃ?ªÖS"ÑÓ?'*'¿ëB?|qض;?Éÿ+¡çŠ?ª~Œé—X64FGL J2039.0-1046¿çzPœ¶À­À<¼{՝VÀ8¹
…"ÿ×À;°¿òɶ˜@´VØ~ܪ?ÿK Íj~?¦I³RR]E?·Ûþ2¡N@÷•p?-<@ٔ媿1¿Õ§D}"¿×ÖÈ#DӚ¿á8ãv\~¿àÓ> L%È¿ã¾XˆWR¿èM3>ñ­WAGNbll3FGL J2039.0-1047TXS 2036-109?ï*€±ýL?"~«—Îó?ZH'¡üÂ?_´	°Lè-?™iª†6Ë?'>T¦3©3?îæmj?Ÿä£¯Ûªâ?lˆl›]¥?x¼ñàwC?Ÿž!E)âZ?b­ÐtT¡?îQ(_2ž$?œQxâý?oΆtæñ?‹Ÿ»öµ3?£†k8ãó?"ƒ^ñ¯½€?í6©ç8?˜÷4j3£?"é{ÍÇê~?p•f"†?³­ã>7Èö?˜¿.Ú<4FGL J2039.3+2150¿çÍÉ)wÀ'©K{(•JÀ:"Ï$•á~À<CN"¸‰@z…Nˆú@ºòDUšf?Í»Ûۈ|?хRdÑ»Ê@ø¸BÒ¨@'ہÆi?ïÿEÅÜèìêÿ½ºá¿áiž)KS¿ë¶
éh¿ïö¦…:g¿ì8ÄL0ZAGNbcuTXS 2037+216?ìØj\?¶v
 À?q¦¡º?)?oTLOçOõ?¸.é	+?µÕ´_É?æ¾Ð¼S§u?Çúγ,û9?•†óøé?™Ê8W</?Ñ)üø""?DžkJJ›??ê?ùµ{Ï?§‡,%¤Ž?¨uñ..wá?"®¡ž'½$?À⟅žrË?¡`>ønLV?èÏX¶«ëz?£‡ÜÉR?£ÄœY"??Vk23‡n?ÇÑvëBQ?¡ÁÎñe"
4FGL J2039.5+5218¿Ãà¦Ñîþ.@[]ô§ÝÀ9èê1ÄÀ<Þ7X@!ž†)þ?üÃPíX]?¹&+¸À{[?¨ˆÝ³N÷?ðcª2n?þ!M:ƒ?ït²ÄãÊ?¿ïüáù?ïöóçÃɿ丕k7¿Øædÿ´¿Ô…qÄhzAGNbll3FGL J2039.5+52171ES 2037+521?áij‡eø?Äx†ºB£?v6ó–Bm?fŒã?ÜLe¶ß?ÄoŠ›áÅç?Ûq'¾OÒ?È{‰*B‹t?¦~/Ù"?˜ïñœ	2Ò?áФ¨2óœ?ÈÍ&­ŠA?çUêI0A?¨!´`?˜WÐՅð?ÿäÜr?Ði×)ÐG?¦ý×<™ÍW?ã¼ëÖWà?¹˜ûE
ó?Ÿv;y.s?™#W"ÀEô?֎ĜNi?¸à°5Á%T4FGL J2040.0-5737?î‡z‰DHÀB‡DÃ~orÀ:+jî‹cvÀ<K¥"cØ@mdõxµ@ÉÚª"?ºYF¾U?¢Ì~HZaË?è¢FçE?õ´k×êb4?ï˜Úϐ¿áƒ]©~i¿æJÀ¾¡'¿à¶}Õî´~¿éâ…0V	!¿ïôÚgÀºAGNbcu3FGL J2040.0-5734PKS 2036-577?î»z×À¢$?˜vªúW)«?rñ{m)‡7?iÛ¢å2?¡ê#P¬Ý?—Jß+ºœ°?쐈D‡¼?´?šØëÌ®?–²=ñ5÷±?Ÿ8ˆ	²{s?µÒÜAŽD1?®'
Ì99÷?ì£qÌ»ó?œ¦Ü}YÐX?–Êπ
?‡h¬Ä€Ê?µa´þæ@b?—5á«àÓ?é!ÜzÂ
?¦/]fѦ?¸ûäî=ß
? |·üëD*?½õ7=Dˆ?Zéê©Ñù4FGL J2040.1-4621¿ÓñiBþq#ÀBкs-õÀ:¶€À<p.½'¬î@ øŠ/nW¡?ùâؼ²£?Å®_¹Îî:?Á¬;ç%?ýõÇèa}É?þ1ÿ§?êØ+ÛPO¿ï痞—°5?îõ«þO¿Ù˜*™0¾¿à/ ×{|x¿Çyœ#6»ÔAGNbcu2MASS J20400660-4620180?î9GU F?¡&IFh?`'ÖA¼é?ZÓ;ÖÛç?«bn
Aßä? —µßÄ7c?î¥]ÿG]?ŸäDÔ-X?aúÓÑýÞ?kMZ™þÃ0?¤ŠrÙÝn?x7Q'zì?íi`øñ†?•ÐõqQþ2?u)ò<P0?c>ù]Ê?³bc®Á?"»z h?ê¾TM?¬‹ÎØñî9?{Uª€m?s}VvÐLl?ÇY_vÈY?¬©ª;Â×ñ4FGL J2040.2-7115¿ìøP@µ&éÀAs–Б}À9èFžÀ<<é•Zo¸@!Ž^I·?úIޚTª?¶UˆÞ
ŒÌ?¬_‡œcoÞ?÷ƒmjW@H­Ù©T?ï§hß½jY¿ÛÄþø*¿Ô;ýÊ
ü¿Ú&æô–?r¿Ô=¡ K¤ï¿Ñ*=áb.AGNbll3FGL J2040.2-7115PKS 2035-714?ìÌ\vO…/?°ù½°rÝ¿?pÕgr?bX£·Y•z?¸œŽü2	?°Æþ¶¼?î9ð)Ç?§¡ê1Ζå?sÛ²[Ó(?'µÉg0áŽ?©å‡i.?¥-uòÄö?ì_Áûþõ? ¾]\ìV)?†¥÷•%+8?zä÷¹á?º-1-c®?ŸÚêŒÊ2?éúÎyª?¤óo:j,C?²Ù™>þý?zØÂó'¥m?ÉÐç,…Ùe?¤¸Ñ"Ûù¸4FGL J2040.2-2506?äN¨h©žÀA4'¾‹ÁÀ:³íضÀ<i"`šu@qàqo@àú)&j?ÈQe£Gî+?ÂOÒ:Ê×)?ñÝ t-Þ@7 ¼c?y¿æ*#õ¨Ž)¿å4¢žûÙ¿çe-BŠ¿¿ïÿËý™ô2?ïý1¹¶o"AGNfsrqPKS 2037-253?îg"zß­¦?Ÿz"Sؔ?tøƒªÛ§?n엔ø÷t?¦ç·Üª+?ž›+àX?íÑÙ˜?§"H{tN?€©ŒO–òm?Š7]lƒ?®Ä[Y	é?¤±æ^÷_Ü?í'"IY<U?"N¨­Rðo?‰`ÖܧÂ?yïtVοæ?°ÂݺZˆf?'Õc›€_?í">žc+Õ?"ãYœkð?V˜;?Éû?~n֌q¨…?®Éü-]§?'$†ò°­Ž4FGL J2040.5-1705¿ì Áè("À?—‰Åæÿ~À9ÇlÝxì{À<.œ×%@™ø÷øõ@l—E+ƒ<?±úëC/Ÿ¿›V)úœ¶&?åçÐ^QÅ@˜gu/,?ÝZr§½HË¿åǞ¢ŸÓ¿è¢ƒý†(¿ãδ˜ù`ª¿â~5ZTà,¿ïÿ»lR8²AGNbcuTXS 2037-172?ïℓ3ÝN?hÇ~ø+?@ÒãEȞ:?9Èÿ~šá?iF³ú°‰ˆ?fÉ퉝e?ïÊ1ëaìÁ?~À±eWr?,Rꬉ?PXjÒïْ?z§¾'IÖ?|¢ÆLJ?ï#ic¹r?Ð8'ò~Y?j}ø>q?YJkÑ?˜LsÒÁË?€ˆ¯]oá?ïØsBZ`?ZaÖ>c¾??¯EQÄ?0Õ-B'©?qÔÓÞzÖb?X:?ø²ô4FGL J2041.8-7319?î¨áfÀ@ÜL˜_À:¯UQk,ŸÀ<•íÒt@ ò¾Íە'?û0íÕ·?È''·ÿá?»Q'ľ5…?ôÓæIîa?ù§zÓZÛn?ïÜCb¿æD¼'Âåÿäµ&Rz X¿É]F,4;q¿à•t;;?q¿Ù^¡IòAGNbll3FGL J2041.9-7318SUMSS J204201-731911?ïrÆ®¦W?†…‡ôF›î?=Þû}ˆ}?5Uãûh"¾?'/Àœ5´?†/>2M'?îvw3N]Ë?¡ÙÎdá)?pÐN*%Í?{€çº\Ö0?¦~ŠÁTÞ§?Ÿø™4÷xŸ?íÏÄDñ@?'àHéñ?rd²JCA!?aP[ÚÏ?°['³ÑË
?'\×xØý?êÉñ¸Ö	€?¡Ñ*w|?"èBµÊ?'Å]2ë?Âf<߃I?¡ž`74FGL J2041.9-3735?·X±÷"O¥ÀBž FÇd®À:qíâÇ
À<j+…¿È@ ÛB±Ux?ÿŠ7/+?»A*—®2¿~À!´(é?ÃG¥NX©@‰}G(ˆŠ¿íÖ±v/?áµü`äs¿ášmÔﱿÛSJÕù¿äh¸@"ÚË¿Àr€óZ€AGNbll3FGL J2041.7-3732NVSS J204150-373341?ö¹i?³®– Ü?Sþ͆$?K'e)×Ì?ŠÓ×·ôõ?€Ú8O~?ï'ÐT'Ë?ŠBÙ~Š?6ÙsPÑàÚ?JöÐõàæ?Š•0ÐX¾9?‰sš¢]÷?î;+ZpS?ƒ¦Ø'ž?x$›ì÷0?fv›È¼yù?¬G¹Ìº¿?‹D£HeŽ?ï\ÑÄÿ'?|ÈacöÆ?l*³Ž?V¶žò'm	?œQÀu©œ?{þ¥¥ê4FGL J2042.1+2427?Íå¡ÅbZÀ%'Ó"wÀ9åÚ rfOÀ<$;¿É¯@ y2&ì±?þa8"œ×?´›m"<æ?'vx_ë¬?àØ¢mþ‹@JÝîZ¿èœf2d[?ïÿ8Yã¡%¿ã7; ¿þˆ¿Ô|_Ìï1|¿ågðßьO¿£a+'AGNbll3FGL J2042.1+2428MG2 J204208+2426?ï'‹\+Ð?"ó± QÌ1?V¬B‹Ú?T4ÏÛ,¸?ž$êkÁ"B?"{ùDVì?ïXY›°O?ž¿µÜRð?Aðë5Êßµ?XlyÍ•?"eW2۟@?žlmYvî‹?ì™C¶WgY?œm?"åu/tä?q«Ô¡³?¸™?^žÖ"?™ø›9Æ·!?î¬úD)?"¬?ÃäÓä?€qÜÖ³Q?j–êþ?¡#«g6Œ?'
–ÉÓ4FGL J2042.6+1629¿ž<{"˜À/*Îî<´À:Ä_½Õ¹À<]JÛÆdÔ@ ü›nÛÕÔ?ûC«Ë]a?Úù#¢œwš?ÈÜ!>6?÷€¬¹1@[K€1È¿ïøŽß#?ïÿt¿Å}M¿èJR]¿ª†ÁáÈm©¿êU8Á'‡?¹%ü"äÎÌAGNbcuNVSS J204242+162910?ïæW	X?ƒŽ¼eۚ?RôN2XÄ?M·1	Kþ?Š'è2·^Ï?'Øwi٘?ïJ˜rv-?'õ
ìÏÙÓ?C?p?]ÑCw…†R?Š¹`âKs?'(]%#Vø?햡\ÑW%?–l›ÊȟY?~'.~
	®?r–Ì¢6?±aÒ1"v>?"¨Ö²ò¦
?ît"R÷¿?Ey'áãó?ePXžfñ8?e}67κƒ?§bµF©…
?#O‹È4$4FGL J2042.7-5415¿ÏŽ6ë_ÆÀBä›A9†4À;G™Ò¤}"À=<ßP]¦@H;®@€"d®ÖB?Ñãz¥vÈ?ïÿûB«÷@FøðAF?÷'ïUÑ?í#Þ¬s;¿ˆÛ^¿‰¿Á–½FG.¿ëŒ#>Éik¿ïÿó€?ÖZ?î€Ý`í²AGNbcu3FGL J2042.3-5416WISEA J204241.98-540925.3?܂ÐõÕ?Í
ÏdÕá?ÞÿÔ¶O?Î)I‹«	?µóiRP=?²VAÜw•¿?Ì07àX=À?Î(-!£ÿ?ã'ÜC/@?Ó
è¼Töü?ÅǨ®›=?Á×Ð¥×Ö?Ï \Ÿy2+?±à¼òi?áB/åÀÚ?µÈwÅ"Ø?ËÖãÉxÊo?©/£Òٜ?®*ø,Püý?ŸÖRCà‰
?ì8ïÒ4¿,?¬"^dP?®F
°cH?£ÎĶ"64FGL J2042.7-0155?é›8ýUÀ9iÂ;ySÀ:¶ãÊ?SÓÀ<_Öñý3@Ð3Xœú!@I:÷LÓ?ÇÐÜ&$?·vi¾µ‡â?ï:"£§@'èYp3Å?îò«ž~Û¨¿ê'ÇÅüÏ¿Ø̟ëÃ2¿ê3oce*&¿×'~!îè+¿èM?£ÙäAGNbcuPMN J2042-0148?ìÁUÉT?ªµg·'?q/¤‹P|r?gåc-6Ò?¸à‹d­›?ªAà'i3{?îæ´5À?š-½Ò•å?c?sÕ9gè?tny"Ö·? `ÅiÐgá?˜Cÿý"±S?í!Ù)Ђ?™e+ppâ™?‡£N¡Y0?|î"è?´Ÿb†Uò?–-7؇V?í̊èÑ:?¬à€/"?rÏߖ¹œ?dìT¿Âf°?°n¸K}ª ?4"€ÓËÖ4FGL J2043.7+0000¿ëãk´À8Â:îéWÀ:oÒ0¹Ü/À<\g=
¨@zî(½
'@n[þ-˜?¾¬ƒ×œ?›ñ"F7`®?àU'"W:@§6ycÄ ?î¹Ú¡÷Œ¿½Î6YX`ê¿é킺Z'¿Ý§]CýÜ¿Ú«zl­¨D¿ðAGNbll3FGL J2043.6+00012MASS J20434215+0001193?ï€ÍH¯›?…2ìë /I?]X)Ä×?R¤'öÜ?ŒÎà¡Ô?"T­'†v?ï…6 ?‹®8;0Þ?=Y«}á?OþP¸B?Ç±:¡Lù?Š$aaßV0?íéZÎTr?"sœŒ•/£?}öÞr9?q"¦™hUâ?­«^ûʊ?'‡1#Ò©?îß
)÷èþ?€u"êÀ`&?pøØB!dÌ?_¢ß¨'}?Ÿà"°z‡0?|€%¸4FGL J2044.0+1036?ïQeәo¨À30%"ôÇÀ:Ìóf"‰À<UcV­Í@8[ƒˆ?曥BDH.?Û`ØóK¼—?ïÿۂr5¨@‰
]Qï@
ÊMó(O¿í.Ýãö_?íSq+¼Fm¿æY©ŸK4\?­(<	E£ù¿ïÿÏ=ÀTï?Җ'ýCDAGNbcu3FGL J2044.0+1035NVSS J204351+103406?ï²\jŒ¨n?ˆÝ­)8Aë?kãv¢k»C?rçtøŒpj?xàhuêº?ƒíqƯ¿Â?ï=Dz¤žû?­a5zuj3?|üuGý`?¦ÐCP‡1¸?'k!l?Ÿb4wF›?ëPÃöHs?¥Ž'"¤Ú?¢¾Š˜º?'¢Ù/pLä?¼ JԈp?¢¨·-sç?îò_ç0‹?™¤'{pÙu?P³îÂh-Q?T,:? Tbä
?™†Moìý?4FGL J2045.1-2346¿îa)¢ÞVÀAm_Eà´áÀ:‰ =!É~À<|µwE²@•òôÿ›×?þéùc-ÌÂ?ÂÉë›ïà"?¶]΁¸1?õ`Ɋ"?ü˜k&ºó¿ïÚÍáŸÂ©?ïûû…Fü¿âµQñd[Ê¿Üè˜DÚÐq¿æX²é̷Կԙ}_QIIAGNbcuNVSS J204457-234643?ïš]›½Ü?€Š!Â@|œ?Gýl‹áv?@zêãÿ¿?‡èâP`{,?€ä‰ÓiË?î4#Û|?¨l¨—'vk?qÜ°¥ƒ?z4.‹ë-?ªƒG¿sŽˆ?§,¹¬[k?îÿ¯+ü?îr°ê˜—?xn³ÂMq?cPˆÙ¥"®?¬Ý·9öž?–‡.q?ìz—Á(–?—Þw½ø¬?•˜Ž:i?»H"*ó?¶Å="@!?•÷qÔÃ<Ç4FGL J2046.6-1012?ä…ÌþÔdyÀ>1Î_pÀ:ÀÛÉ¿ÒÀ<sÏÃøõ@ 33Yæ?þ†ÃÓÿÆõ?Å!#ü‰}î?³Žç á?ëjÑ?MGÜ?ý¸]ϓüw¿àDÝ¢x?ïøðâUË¿âó[Ao6¿ÜD""†ã¿Úþ;¤ñ¼p¿åa8^ì¢AGNbll3FGL J2046.7-1011PMN J2046-1010?ïYd^³âa?Ù"ãxŸ?U§ #¿í?VdªÃT?"ƒY·wÀ?Ä*½w?ïNA=8Êa?'¼h;ÅȨ?IwÌz("û?Sü-Þ¡â?•lõoX?'?+¶ðsÇ?îƀ"Or?^&ó¿c?s¼ásD#?]ëÒr€-?¬àà[Œ V?
éÏ¢ý²?íߎ ¸y?‹|X›?€Û³	ðA>?lo¶óUy?­Ð13¨h?‰+‰ê®V4FGL J2046.8-4258?ïþ@Vv,ÀCXœM©?À:Ö0Ï«¤^À<"üæp@>M(|ËÙ?þ>O%ØÝ?Ï]JˆåAc?њýôþ@:'FK@
ٝëØ¿î·3"Hø?ïý̞ÿŠ¿ß;!`Lò¿á9ýñ7¿ê]ß3á¿ØâÏØðÇ~AGNbll3FGL J2046.7-42592MASS J20464397-4257134?ïç^j€?ašT[>ۆ?C®Òžœo©?;­Qº ?cöìîXe>?_–šbÿG#?
Eà™?‰ìÚ©ÐU ?B³ô"/Ñ-?Z¡Æ&´ì?‰ò=eTܗ?ˆHù–Ú?í†Àíg°£?™¼øÍÎ?•lܚ4?‰"
 à@?¬Ýã)¨§?"õj¸·ù?ï‡ ó¼h8?q0–­¦}?_7,'¥ê¶?NM]ÝMT?ŠP݀'4L?pé`4§74FGL J2047.1-7400?éæÇâï#À@ì4~ŒÍÙÀ:ê»±òUóÀ<\{Xeò£@‰)Ô½\@Ü0ûJŽš?Íb@<??ªzK[Ú,˜?Ù0ù½EÆ3?ø¸+Ë	ÿ¿ïhšˆ¬âL?ã"×/Û¿ë΅¿G(3¿ÕµÔl©¿ïcȑԩ:¿í¾ÎaÍOAGNfsrqPKS 2041-741?î¥MeîÖË?¢$pñ"?nh$ªiu?p%ãâ"[æ?£ÉÃÇì¹?¡Wöh'?îÁyXª{?¤æˆ0#:?lnŠÁs¬p?}´@è?¢!…~^ ?£@%‡ö|%?ìËÆfG¬É?•iŸ©Ù?'á-cf?"%{gNÖ?µ)†‹÷@Ù?™°íj¢r?îbMh¥çp?'¢wF?5ù÷ßÅ+?ôY
Ì?¢
ª÷©—Î?ŒmÙ[šÎ4FGL J2047.9-3122?ï`ýMjŽaÀB±" ³Ô®À:bý%Z-À<køIRYi@jñõ%["?ÿô½±§?Äݑ€›pß?¿2&˜Æ
?úMn³<@&lXÁ?ïüšà–ƒ:¿è"@¡°¿Ü$.³q±ô¿Þ$)ªô4ñ¿áq¸¿y¨
¿æ^Ê@*'{AGNbcu3FGL J2047.9-3119NVSS J204806-312016?ïtE›<j?¬ÍˆÚb.c?{Ì ;"Üä?­o_¯§³?…Ih·?yÞ·ôÉtA?ïBrF\B?"'ÄOi?IÌ08«6?VFS§*Y?–èØݲr?'l¬]¹?î$ø^
®?ã­RùáÊ?p¿éu·é?ZÑ·gËî€?«˜|ð´g?Õ1øÚÉ?îMZ°§U?…Œ°al/'?ne쁝À?XË+‡ Üù?©Cö40Ó?…=ڟ›À…4FGL J2048.6-6804?ïÒ2t=áÚÀAì¹w…r›À:FNEÞ1À<w3Ï:eW@[9ë3?H@êùÞ}Ï?ºÃ¢Ÿ¨?¥4V@Jë-?ìŸóOîU@'Le¿ïü">`¸Ò?ïú³ääò¿èbªºSM…¿Êå9ñ=o¿åãflE£x¿ê.ՀzŽ¼AGNbll3FGL J2049.0-6801PKS 2043-682?ïåﮖæŠ?b¼Ðw"R&?<۝‰ç²#?5ÓøÀ¹W,?ftÝ·Ü?a8"™é|?``¸?-•­…X?G!˜OΧâ?^3aaýW?‹jÎbâ§?‹"¿ü+­?íÈLê½ë?">ZÉ¢™?áIð?sðêHd)?¯ßID?'ž›"£âY?ïVP'ñp?^ñ»'<? §R€¯?rQ¡Ìh?Š›Ùð#Æ?u0ú‡)À4FGL J2049.0+1647?í­vµïÀ0¦ˆŸsÀ:¦ÖŽín-À<C瀭9Š@,»h zÊ@¬Å@'H?ß;Äý ?—ñ`CÑTá?Øó÷ÿ*˜@	è	ê§?îÐvoÈå·?ï˜þý–ï¿ãÿ‹Á>Ï¿çWÌ'ãt¿ÖâénÄú¿ßq+{ÙÀ%AGNbcuNVSS J204902+164727?ï1íæ:¸?1…gâ?oØӐ˜?¿?iÇ[Á¤?•Ç(Ɲ?&3 .5F?ï˜ð®ç'ú?‡èßÉ"2?>Âà†íMX?T[lÉ£m?ˆÍ½Aã×?‡V…a(¯?í¡Aìæ?™žÖv¥'Á?ƒ}·ÖgGÇ?qtÏÊ'bF?´ë>üó¯Ö?—«L܊Uf?îp#™6?ÖÇèý;è?|B)«ìw?rV€Ä1?¥zž)J??Œ@áÇÚiÍ4FGL J2049.7-0036¿îט[)ƒÀ:`Æ÷ µîÀ;ŕ$¿ÒéÀ<³YÿOÖØ@#­ieIZè?ø–þ–µº?ɺˆç𔨿¥L9iƒ&f?Üi•ûg¿@ßÇÓ顚?çFyáîG¿ïÿþøþ"?ïÿÿ²}@?Ä/Mu~²8¿ïþø?ïñ"b"4AGNbll1RXS J204921.6-003930?ïèt=e8?d¬i;y?1èI·ˆAs?3¶'V@ïî?eN¹¯©ÀÛ?c5¶#g?î徎ÿ]1?£C"«/"?^щ&5D?r"QP9¿? ­ŠÆ؄l?¢co]á,¶?íKPj
 ?—ç& <ª?…t¨8R§?€dcÛÙ 7?²ö稚ÔÙ?•äÉc>®?é?rÁQŽ?µ2«ø?sIqk$	Ú?w'jqx?Ê𶩡™}?´ø®n'I¢4FGL J2049.9+1002?ó<À4µt'yèÀ9FÛeNÀ;×/(·Ä@ÙƐȐ@'£}H*;?±âò~Jf?¸)ÙBQ@
£ì¤©(@h©ÿ˜Q?ïøkK¨tÿ¿á­#ŸAyG¿æÚw_²íþ¿çL£FÁ…q¿ëC®á){$¿ïþh@0FÅAGNbll3FGL J2049.7+1002PKS 2047+098?ïËi³½š?‡± ÛÅì?dÁœax?bqÕ6½Ñ?oÔ°*kÕ?†âg­'yí?ï‹àÜy‹?R@>ìæ?U÷ü^•?m%~_Ž^?ŠHÉUöêa?9?Bë—A?îÆSq'ý?aûÀ+ý=?"W ëí‹?|ÍÜè-Ý?	½ÐÙ©¥?…ók\Œ/?îËæ"Lâ?½kê8ú?†ÔÀé]?r	l^®&–?›{áµ;?|)Œq?4FGL J2049.9-2453¿ÕYË8ÀB¶â—À:úÎû{6À<_ü@WÞä@´wWû>¥@nxžwNì?ÚÅ>c?â öàqšL?ïH'AÖ@xh"<]¿ïO>â=ø3?Ô_ÀÚÑh¿ÓñS)rÀ¿é{'¾Šêª¿ë{H`A^?ºdÈA!ÞLAGNbcuCRATES J205011.52-244811.6?ëœ6=Y1?º÷|zŒ}?Œ¦*­é¤y?ŒÑ`b»àÒ?¿Š¸øXë?¹bÑ-Û§S?e¨©?¦"Üÿ™î?xÿàˆ?Ž÷†hÖé?¤‡WŠ$[? ŒE_êV?êäž'L0?¤=T ÿ?ªyH†«p?"Â5/Ø?»žk€,ÈÎ?ŸPÛÂ÷x?íë­±INJ?"ó{A\?nAÉW'?bP9T­Ï?¯d°ÎÒî?'ˆ˜aÐ1l4FGL J2050.0+0408?ۜ™Ïۆ4À7ùb¿ù'À9r{'pÖ,À< ¢ûB+@\Ø%ñVD@BÌ}òt&?­I¦èÃ?qßKäâ?ÅóH6¥ƒˆ@P5Þß?Æ{Pða§¿ãOÅx¿å›Èé}±¿äb\¶º;Ñ¿Ü]/ñ_SM¿ëçZ¢bëÞAGNbll3FGL J2050.2+0409PKS 2047+039?ëïáMË?´L^"Sœ£?uõOÕ´?jñLèÓ¦?¿(ƒú­†h?³å§KlV?ï¤MØà?"{Êíë,"?<Xˀùðb?NGæÑx?†	Ãkô-$?ƒˆ"<àä?ìÑ­^ÚÊ?¥¯Ò8Ô@?©õRiü˜?8«Š²¤î?»D3ê»ê?£ªÖ]l•G?ïN'íDÙ?|kJëVE?qF'%nU?_w㩶ß?'Ü8'´ÉG?xhkŒ
äö4FGL J2050.4-2627?ïðn9ïdýÀBbBAÃï®À:)ÞÊü5À<=BùyÔ@"»ªŒÖ@skd?¼‡¾ºÌ€?ÆÅÓ^a_A@
d²ú"¯u@‹j:±VÐ?ïîÀ!ß'¿Ð'9@=‡Ë¿ãKÈUnÇ^¿á."2Q‹ä¿è|J°j¿ïÿúâôAGNfsrqPMN J2050-2628?ïõzwñ‡Î?WR?†©Õ?Cƒìç™x"?L9:ÈÆs?F'3RGKì?EÞWâ¯~d?ï°K™´—ò?‡[~Jò°?6!²Ñµ,?Qðǂ>þ?ƒ<üL[á?…Æ\º("á?î§ýãì?›'L[µ?ˆâkðÛ¬?'g¢ä:ò?Ÿ
ï'™?ƒ›IÌñ?ï¨W"¿T?k¼ø?Qhãä ´?ASY)ì?ƒÉñÞS–à?i_ãÉ<¸4FGL J2052.2-5533¿ëËaè¨KÀCÇÞP'ÏÀ9M™æÆsÀ<-º9LQè@}»ÏN‡M@
hn~bÜ?§$H£v«ó?±ÒbŸÃý@$]È23Y@µ9"÷ƒ?ïÿ…]S˜¿ÛðŠ!«¢¿äÖ¹µ˜Ó¡¿äf;Óë¤ÿ¿æßyýò߆¿éà CAsAGNbcu3FGL J2051.8-5535PMN J2052-5533?ïÖNî~p?jò‰ðV®‰?)\ˆ:÷J<?!™ÉE}dÃ?t,tFé
ä?jtVw¥g?ïßãOš?'ô^‰û?0•Ñ΋çx?O~Šæ@÷²?}&±;ŠtÚ?.TH'M.?îç?ÁÜñ?†òs»7:?rùˆw½y‰?gÛ=Ô¼¾¡?žY¥¿už?"—N$ºÍ?ïöX´a(½?Cã «&?$÷§ÐØÏ?-T®ªËè?P¯¢C«« ?AϨ'ÿ•s4FGL J2052.5+0810?ÛÌX¿oþ&À6H†zØä2À;Ӆü-ãhÀ<ÔÔoX}p@#­w§Ši?ì6q¬?æ\-Þ	¶?ïèø5u@Ä	_$RÆ@Êmˆn£ø¿¤	àmW`¿ïr}šàl¿ïj¼Â´Ž?ï÷V¾}©¤?ƁWƒt"¿Ñd§I……AGNbllRX J2052.7+0810?íøi|z":?­×—rz?†ق¦S÷?"Ú¨Ø/ò)?ªøq×®'Q?¬}= DkÀ?ìÚéѱ'?Äë‹.sF?˜¢‰sÀ ?´"Ë*Ñf?³n•ƒO?ÀPèz3?ëî¾£‹-?¢÷±?
?zÿ'U~Î?'S5';ÛI?¼kKîFæ?¡Á˜Úö N?鰝ýÌiœ?¼öWà[š?s+mÅEu?˜¤Šî"?Ȥ,š¤-é?¼@P03"/4FGL J2053.8+2922¿Ý°› §LWÀ#´§qÉpøÀ9[¡ÔÑ~À;½Ca~ @ ïû_‡O?÷7קò!ñ?¹e1³rí?ËcËV€b@ÖKìgœÇ@	äQ»ßi²¿îâ/àm¿àÜ ý¦‰l?мj^ÄпÂåр´¿Ù1:_¢Qú¿Þ³+;-CAGNbll3FGL J2053.9+2922RX J2053.8+2923?슩úÛ	Ã?¶x–{aKª?"E|	N2?–#°6ƒÖH?¶ÙQ&à^T?²é÷V€Ù?ëÚ¦Øì
?Ãð¸CTVð?ƒ-"tÊl?ž¾ã-b‡?¾ÅÊP?Ã]·ð°ó7?èô(
ðË?­¤'qüB?¸¨Žû¾Æ?¥.â?¿¶0¬ºá
?¢2
™¶?æñ¿lá©1?±3].R˜?"ýo)Ë?tL`aà"o?яàÆQ4O?±UP4FGL J2054.0+7024?ʂtËL$@0cجëÀ;½¾<RÀ<L™iÈñv@ 
<ÿdÐ@í-zŒŽ?ÅÀæå|Ç¿èhV"ú?ÊkÅJøL?󏐬5'ª?ïâp½Ø=C¿ì€"'‹á¿ÉÕ`ÅÂu¿é"²a'•i¿ßdIÁ1濧ÔŒ:
"AGNbcuNVSS J205350+702404?ë¹wbé?»+vr	B¯?"b*ø	²&?ª?@?Â>ù¡Ù:?¸z…ö¶?觫éBž?È)ˆ{Õ£ß?›YµaøÙ²?ªž@¤tý?Éø~¤ÚV?Ç0Fk"S¨?ì
>/qg? ½XéÁ
Ç?¥Ü'JĄ?ƒõÈK<ó*?»l—z¥3°?ŸlIi?㔑yù'E?°´wSçë*?œ™9ÅO	ô?'pvW h?×
Io·êÖ?°ó.@½$4FGL J2054.5+4731?ëò¨¦Ò½'?úG-ÉÀ:|sÁ˜¼$À;àý÷Cõ@"
d|¬Mü?þÆ*\}?Ì1°|4.?¥&8à™?ØÏ1Ì*æ@¥4L?äæ†ý_¼©¿Äè'Ç¿ï³Ü:þÚ?äc=¬ˆà¿àւ""F¿äØ'sâAGNbcuNVSS J205432+473338?Út!Ðs?ƆzÇ(§:?€bŠßÃç?¢Qdcõ^?â"kƬG`?Æ©ŒwÐ=›?åpĝ©ãï?Ж»}n°ô?qÏ:Öf§I?•ìÓ¹¾.,?Ô×9ÙR†?Ð~Z-s?ãÓ(?±üðŒ©lY?˜y8¬á¢?B",Üë`?ÖÒg<]
Å?±ˆû>Þ?ë"yµ«ý?®³ÈY.ŸK?'"·Û×?EFÜr"˜?ÀͯûmÒS?­û4±3³4FGL J2054.8+0015¿Ñü¿¤ÀÀ;äÚ	Ì2À:")¦ÂwÀ<O®‰ë¦­@!GáõRýÔ?ý!þ¨+¡?ÀY ãOp¿o+'\2¨@?²H`þàì@P¹Qð¸?嬗moo$¿ëåáℿÅf˜egÿ¿Þÿ²þ æ¿Ôâ5_wn¿Ú¢5_wnAGNbll3FGL J2055.0+0016RGB J2054+002?îç;=ǎ?˜Q3R',S?[ @Y²Õì?W.ÿт€? ³LùUðZ?—'œ"r?ïO ¤Ý?'~*³ƒœ?IßÁ¯+?YˆÎìh?•S./ÝO?'Ë{ÖÆéq?í8%™´É?œÔãÃk?tQ©§ðœ?a#À¹Ô¥§?µÉ&¸—Ú·?›^ë"A=7?ì¦1š-ÞÚ?–ûœùÏN?cá5D'_>?U*
N¾å?º/i"lö>?— ³bŠ14FGL J2055.4-0020¿æX'´èLÀ;sP]¥À:F0l¯UÄÀ<<¥5¯@ ê&dä?ûäÀ>Ië?ču‰nÿ?´wÀÁP»?ôô¿%D]@Lyµùw¿ïܕ'2Ê®?ïú«bùÌ¿êRÆ«ú?±1¦@F¿àûã:Í[h¿Ù·ÿÛ<§AGNbll3FGL J2055.2-00191RXS J205528.2-002123?ï;ªüY?'¡û;ÿW?JzOu<?Eãî,Í>?—ɸD,ÌÈ?'X}ÄST?ï'qúÜê¦?‰i²xÉG??rÆâoá?S8ÀÕ8ÞÚ?Šjí²ŽBÈ?ˆƒÐ¥?ìŒk`ï÷? FëåôŸ&?':r4°'?rÓùêû?¹UV´úp	?žX¨¥ÿ˜?îO%©¥f-?'ˆ¿;h©?tÍáÌûLð?hõq—±¼?¨sé,
3ž?'ðè}4FGL J2055.4-0504?çjõ×)"pÀ=ÎðZpŽÞÀ:÷ÀªšëÀ<˜ëô°@•\­€k@ö¤¼ãJ¾?ÈWûØð?±*ð¬IJ?å¨D€b'?û/3÷Ô7z¿äûÎã''%¿Û•ýÈX¿çk(½Žkh¿ã'ßx ûŽ¿à?¾øMÚ¿å%:|CGAGNbllNVSS J205523-050618?î¤ÑƒýŠJ?˜bÞ?«K?XͱÆ'ó?MÇ=«Ýƒ¿?¤ìz1÷J?˜$¶áH>[?î°VtNן?¦ãÐx¾­?[KÃäO[Â?gc˛ám1?¤ :›ð(?¦Ÿ]ʔP?íè&ر']?'šAzF=?€!ÌÛ8?ln¯Îƒ•?­uLAß#k?Ÿ­Äg?íÊI;T>?"!‹×í?u…@{…?fh·¬2?°Ub&\N?'yþV464FGL J2055.8+1545?î˜?ñÿٌÀ2"f¥P‡À:‹Ÿ_¬8À<>À//˜t@E'Äë@¢e㉧´?ÌÕY8U†ð?˚KäÚá?ü=W(ÛÁ\@Rr{r'¿áëCII?Þîs恩¹¿çÆIƯc¿çv?!}ÿ	¿ïþadžæ
?ïô€ÜqAGNbcuTXS 2053+156?ïÎ[Ïè?rΘq-?b?}¡»B?dW`‹†™–?o©'vB5?ih0Òn@¶?ïÇ9ò¦¦?œÜÕ¹X±˜?dÇÎI%?sžvx@±?™®5çâ
'?ší%U
3?íò6€ÈF?•YÉÃÚ?‹eÂb7Ú?€A'*Üá?ª'gm­¼?°8b¸J?îÑݹ€œ5?†ì‹Fut?~'u_I?n>Å1€?ž«ŒT¹
?…0Í°7LŸ4FGL J2056.2-4714?ç‡!‹@ÀD1&|k‹iÀ7Š8|HOûÀ;"K}¬Ô	@k?jyž@ÒΤ=aŠ?"'p€Eµ—?»|ûÔ!Tä@"Ô¦°)(@Â*/ÔY¿Ä>ŸøÙE+¿â›SíNM¿çX'AƒÍ¿ça''zï
¿é‹¤ô^¿ë4ÑΔM)AGNfsrq3FGL J2056.2-4714PKS 2052-47?ï…%úX?²î­õ*?p®Ð X:¼?}¼
¤z?š§8§ÆF?±~}«‡Ô'?ï)P]äPŽ?¡6Pós?\® "ËÍ?nƒ!eˆ-?™yal¡? ©1gcÖ?ï
¡[:h‹?¼ì,
/?ˆ;¯ÖŠYÛ?†BZ8@?'ü­mÁï?"á,;Z?ï܄H(Vª?cVÿ<ÒÎ?U"òmô?PÓKg$?h³u^žŸ†?^£~.°4FGL J2056.4-4904¿·l¸Ÿu$ÀD)GA1MÀ:Õ¶;ÏÆÀ<IjÃQ#@Q/@4xƒ@QÈ"n·?Ù1ŸY?î+hߝâ?ÿoœp
¯@ñËß¼é¿êå¡z8«B¿Åö
³¸(Ñ¿é­VN¿í3oce*&¿ï齞[ :¿îíÑ9*AGNbcu3FGL J2054.8-4908SUMSS J205613-490415?å^˜5m?Ès×ê
?ŽzÀ­«Äæ?Šs{~®#?ÔPÅb7?ÈT ˜¢R
?èlŲ::?ÅLìróß?µø_äKC?»Ù´ß¾Ü?ÃP»·Šu?¼9J–úIt?éZuÿÎaÔ?«³5Þ|š;?°ÀíÝ?™–ÙöÈc†?Â6&
EõÂ?¥{q¬›ž?å¯Ãö~Í?¶´zH¨¥?·Ë}ÌOÝ?«¼9BMô{?Í^E±?ÜÞ?² ˜]U£—4FGL J2056.5-0202¿è™QgÑ qÀ<Ž¹¡vÝ­À9ç
›dtõÀ<:"ŒòÂ*@M@NN†@‰êdHR?»äC`ýÆÀ?À¼Ÿ9@>@ ¾×@Ä@I'zìZ\¿k
Ñ¥'¿ß*m¼Æð?¿çÒ·'¨ä¿è0¾yLòø¿çôÝøn;G¿ðAGNbcuPMN J2056-0205?ïݕ1k?j>›ñ4'h?HY8ì	µ	?Cïô³¬?lT€±'}Ç?góð»ÿÏÐ?ïeÒó¶Ý?'Ï™WL0?Cy¾+ªn?]"ždÊ¿?Š®ï`W¡|?'©ÜSrr?ïTw8Nº?6®þr¥?q\8Ù-¦?h¯3ÿ	Í?˜>oJ¿Ý7?~E~opÛ½?ï0ãùfG?qxÎ{b:?dJ'Ƀâ?PƒŒ^áL?‹2t\ô
\?o—Q!$í'4FGL J2056.7-3209?î[68'ÒÀC¯!JÓcÀ:ŸZ·ÜzÀÀ<G{4SÄ£@ô¨^•@¤Ø&"»?ÅûœÙj?³Úx±íxi?äú›qàíì?ý¨å|qÀ¿àh)µ/ë¿çóÂâæ¿äŠ‰Ü¿ïÿÿÊPË?ïÿçÁŲ§?ÀÍ<HۑAGNbllPKS 2053-323?ï™`äãn'?'{Ñ-Ð
?@Ó]Ý9W–?D`s*Rÿÿ?ˆšéPÆ?'^"øžÚ?ïo"O€y?¥É~.%½?jÚ£á}´§?ˆ åÛtÛ`?œ¹à:n?¡Œ°ílz?ìȧŸ~àF?œ¹ÃžÖÇ?ŒÁ$¶|\?' EÐÔ~"?¶:jßr.F?š€S¯"ˆ?ï©Ã>Jô?€A>Þì? ºüR¾¤)?*½Î­`IÙ?…LD{÷ÿŠ?€!j®€¼4FGL J2056.7+4939?ʹ7¢6SØ@	<"?¾À8c}}Ú À;i!Æ#e`@!p±E\Öp?ýMoõ[aP?¨³"?ãDÞ?¡=¢^6?ö­§%sW@	¦"Ö/?Þq&þòcà?ïð¦%™½¿Ëä¯A¡‹¿Û'$l ¿à]*"As¿Ô¾Ô;«ýŸAGNbcu3FGL J2056.7+4938RGB J2056+496?í`[r?¯O0†Ïã?a"í׶<¦?blWˋšÒ?´pˆ]®V?®¼9c•Ò?çüxºÐPÏ?ǪãZµk?_i?›ƒ85çÿa?Îø+4=6?džQDT?è­\êh?¯ú:Þ&x?¢€y³?…~¶=`Mù?Ë7J}ÿu?®hŽä,§?闘Ó6Êû?¬ˆ
P‡ð?¦Ð/åx$¬?"m«ü²°?Ã퐹ÆÊì?¨`ÊØúýò4FGL J2057.4-0723¿î¶¬0Ü'À?P]…TÖÀ:'%üéË
À<Eí@
@o"&¾Þ@pHðŽ?›™#'"?ÁÉÁÕwì ?ùLÝF—"@SãÉ®¿ÏºÆdþ²M¿åëðž¹2¿é(ôëÏÇS¿êîb›Ö‹¿ïë[rž¿îߋ€Ò"wAGNbcuPMN J2057-0719?ïÏ×Ç7°Q?}©[V?UNœ—¤4?ZFÉLç˜?rÀu>C®?xË£gäï¦?î~CÄ)?§vìÚ?qAHŠé?'ñöä?¥÷ەÝé¯?¤(ný?îõ¢™Ò±?ˆØ™þE{ê?qä'÷)B?c¼%lL|¤?œÿòˆ߅?†šú~dÕÙ?îÁµ)¦E»?ˆX‰4–‹÷?ƒ~'"`­i?p»BP?ž
†ñç?"wñ¦"¼Þ4FGL J2058.8-1442¿Ú
mó‰¶3ÀA`Ľ3ҕÀ;#jęødÀ<˜dH~ôÓ@ ¬ˆ0½7@u×ÙôÓ?ÄrvŽ*¦¿«;Ž÷T4á?æ!EÊål?ÿ'g΀¿ÛÔñhˆ¿äpÝî]@M¿Û%⽤檿ۜ–ƒå}H¿â~äw
}—¿ÖH'¶þ.oAGNbcuTXS 2056-149?ï:ÈιÝò?ž$Š?R=dëŠ7h?FÔRhÙ2?—ƒÚžL?ó;½«m²?îÁH2‡›N?¢ÍœH#ØÅ?UwQ1¿®?b"8J,Fç?£?ÂMøMœ?¢ ÓIJ[ ?î\B|žÉ?Ž¡1—ª"?pª˜]6JÓ?]k8t‡?¬è̏J&?*›ÃÈù?ìy³$f?›¶ûPÎÖù?sBkKÄþ¶?dü&8\?ºþ@*ÇDá?œ…™DŒ4FGL J2100.0+2103?¥ÉÇû$û—À0#æÿëÀ:‹DÙMäÀ<(6'cDs@1Þ ôp@Ž ¤»5Ì?ί¹<:ï?ÀâÔánD?õø¶DË,@Íé/.è?íÿí@_Á‡¿ë>"E]¿Ù ²ýî­È¿ë€ y\¸¿Ý»lb&¿ðAGNbcuMG3 J210007+2058?ïd=žÁ€m?‹«oÖe±h?QÒv~E?_֟Œ5¥s?'g˪¨Š€?Š¾È…›´å?ï01ã>\?™?qþ
4¢?Y6Ÿ›ÒeL?l-§ÛWº?˜fd	Û?˜´êþ¾Î?í×
ôl¹?—azïË÷E?}øQTç,?zü5áÓW?®ÐFŽ—%?•雛•?îS.2ÒÛ*?ˆQ*€H?[A`¢7S?M"É	pº?©óÍÁ»±?‡úóÕ;¨4FGL J2101.3+0912?ÚZʨý‡!À7ƒï(Ag©À:ã´+W€À<v*¦€2@ 25\XF@ÍÝ|è‰?ÁI¡¿¨ä;ÃS?åž6Kìg?ý¿SrB舿èÊ(­ž3\¿éãîâvWJ¿Þܳàֆ¿Ûú\}‹Ñ¿á¤TÞ~¥ø¿æÆÂâh?"AGNbcuRX J2101.3+0913?.zJw?ÿ‡ÆâÌý?O<y ë,X?AÞrQיÔ?ŒålÇ^¯S?"s&î?ï24@¢3Â?""ÉLŸ?S¼Z¿«?t(Æ<<¯:?˜}·6k¨?'þü à,Á?î"³ÝP/? 0e-ÿà?rp˜ØB?\îui˧ó?«'´Ü$Ô?›ë·gߏ?ìä^À?˜VQøØõ?v!F1ç¿?hŒº-C=G?·}à¨Óƒ&?—ù(	Ì$Ò4FGL J2101.4-2935¿ïî¸Ù0ÀCï–AöD•À:pÜÀ<4!'÷¾é@ìò²°@Ƙã'4p?ÂNÙ¬Ú?ÇRÇ%Ãß@.Lÿy@
朌h-¼?ëR¼ÐÖFÉ¿ç.÷™ÿðç¿êí3¿Ë¤¿ç¿jäz¿ïÿþˆ0»Š?ïÿ¥ÂqÕAGNfsrqPKS 2058-297?ïèK¿˜cK?awè¤'?^v.÷Ã?[½ÙaB¼Ñ?QcmY
s}?MiŠ‹6Gü?îjjÅâ%˜?«;yÂ?ž:?v¨B˜›Ô?¼m`¢
?¦"KNÍs?¦FüÒ´Øl?îɘô‰á?Š–±whgR?€	J‡Ô6?t•O•Æv?ž×§"¨Ÿ?…º''¬ê?ïA¾Bäö?'â/aîg?sý©ÚGÆå?g¦ø©8ü?'ÈÍ,ÏMI?€[éÑ^q4FGL J2102.3+4702?ïþå}³+?՝ò#žjºÀ8¸lD̹À;9•zP(6@Fx M'{@'ï[m ?´1[}æF?®ú	pìý?÷òZ
7'g@¼¾"ºêø¿Út_Cý?ïþdž;îÄ¿áõ
=€>)¿ãmŽä3ñŸ¿ã´ =¸g¿åálˆ€ÃAGNbcu2FGL J2103.4+4706MG4 J210218+4702?éfü€L?»-Wþy@?‡¢]ÀeÁ?ˆ_aG?Èíž1ùZÁ?ºÓƒyúV?áþ3QÙ?Ï5`2[é?ˆ·6ÛIóô?Ÿ·Ge;³?Û>âþL?Ïæͯ7T?àÅi@3×?µ>tkã	?­šš3Î33?–Îe'9nñ?ÚÅ¡çÑë?³‰èœÍok?磳t‰$â?¨›õ÷,Á?°"ų`*h?™$Ç9ôJ§?É_ÏT+WE?¤A	–ƒEÌ4FGL J2103.0+0342¿ìZñ"ǺÀ:îÊFà!À:j;4¦À<=EŒÒ
ú@e`ïYÂ@¡¬Wâ?%?ƒo‹©?­Ï‡Ò?å—?¢,e@౫´#^¿ÜqÃL¿ä¢C çU¿æþ½c£>¿ãÛT"¼'ÿïnoês¦Á?é|ðKWgAGNbcuNVSS J210301+034411?îgC ¤ˆÃ?£üöžœåð?sög«þ"?jèQ—Š´?§
7±ˆ?£)[rbŽm?ï›ËKÐÁ? d)8 ?Yy-²Ï‹?kÚòSŸÊï?›Ôó»Xïn?ŸX^üÆYR?î‡ÿˌ"€?''\¾Œ¨?{оFk?p©Ãb	?¤I/nå?Ž=úé }?š.?"ò' 2Œ?dWØÀ!Â??Um5·Zµù?œ£t¶Z?ƒàX'dm4FGL J2103.2-2114?ÚrY¬Í0¨ÀC•_x5œÀ:ûXª¼ÍÀ<Ó׃	4@sS¶
"'@U>S!æ?È¿4ïb¤?£›¼£M¼:?Ûj•4°
õ?ý¢ë$PÂ:?ï?Äpݸ­¿æ\IÂkÊÔ¿â%!!¸·¿Ú¤±ÛYØd¿áœ?':z¿ïú"á%Ê?AGNbcuNVSS J210312-211216?ïjý;.–?ƒ|::z"¡?NÐY`öi?DW·Ä¹ñÕ?'©ÕÏ;•™?ƒÖË)}Q?ïðßÞIE?"¢-ªyìT?RœpývF?\1͸¼²?Xôf_þ?"ðYL ñÚ?î$ˆÜÉ?CF7~–»?w‰z@r£¯?fUç"´§?ªÆBëÀ3?‹¬WW?íµ"uŽ)ç?Œtg–»—?y9"òž^Ì?dƒ«Ôèóv?°ÃTdÊÖ?‹=j£½4FGL J2103.4-7816?ì™O"4LÀ@'óÜNôÀ;ºòù‡?ûÀ=Wg:¡¼~@M°À§¥v@,—½÷Fô?Øü>ª_º{?ïÿÁ¶ïö@—»=XP#?þΚ,f?ïغadw¿äz7i"ÙI?à)Ñ =ô¿çÍ˚¥˜¿ïÿßéà
¿ïÉöž'ašAGNbcuPKS 2059-78?ëô•o+5?¼æ¡ÚEq>?®;‹úÌ.?°´›Ø>?´u½Ž‰@C?³,öĐ?Ücÿväº)?Óhðx+I?Øsgá?Ӗ_­T2Ã?ÇÚ+fÈ­?Á=ß}—KG?äÛX?}H?¯ž"Äå†?ÄV³tÖ?¦ú[/$?È;ìš–?¤í–¬±Ÿµ?Ѝ¹]¶Q?»lõ¥<)?ä],ÌÝ×T?Á¼¦uU ?ºâZ³šl#?±Ù¥x44FGL J2103.7-1112?ï"µjc)ÀA4Z¬1À9ßñQçSaÀ<hdÓ¿/U@ÍB§šcC?üŽ`¶#=?¼¸KTg?ÝóB¢'åÆ@ @9«ó8@r¤íà˜²¿ç7àìêO¿¡qëCŸ*í¿ËJl_Ϟc¿æs?ã­¿ë¯eŽ$Æ¿ïÿœ}y¨cAGNbcu3FGL J2103.7-11131RXS J210346.8-111335?µ…ò+¤Sf?°ˆC*O5ˆ?ìW~bö==?´¾³cà·À?žøjò§
¹?žp¹øÀ?ÆgÄsMT3?Âœ"¤Z?å¥ÿAS?ÈW{-?Œ*?Ã>‡d¯Æ?¹'ĬzJä?³¤úƒRÝ?¢u‡—LM™?êÆles#?¦ZæVàh?¶'¢Ìã"I?—‹å‰Ìå°?Þs¾›?³~»Ñ+ú"?ÔOE"%@?³ŠsµJ!Ý?ËÙ>Ž°8E?¨!W-ìtÿ4FGL J2103.8-6233?îy–ŸÇ¹›ÀCyÅoÀ8ó¤>aeÀ;éµ³¬@wèºéö?ýº›
7 ?¦¢,+ܨ?»¢é#šŽâ@¯.Ìț@
{H!+ô¦¿Ù/F>¨²;?ðFyŒ¿ß¹õ¤ÝD"¿ßêoŸõÿ ¿åU¦$ÂW(¿àò''sã'AGNbll3FGL J2103.9-6233PMN J2103-6232?ïÁ—øXb?sÊ'SÂ?OTD1êª?Jµ«¥Èè|?{I{M'Ÿã?q¢û,\.?î¹E
Öú?§È#Ö
?mwƒ8ïð#?}opG
b?¢˜{Ñb?¦ÑàíŸ?íŸ4U¤î?¢§™ù¿'d?ŸuãÚ¯Y?–äê@™È?¦‰ÿ³Ò‰‡?˜´%wð?î"&Xèm?‰ÂMMCf·?'Ź$1b?pÉϳ.‰ê?£Rƒ5<Ä?‡:²<ï4FGL J2104.0-3546¿Y<$‰zOÀD´%®æ1ùÀ9Ì "ˆÞ`À<FŸ°4@™ãtÙñ£@ÁDÙMä?³·»B¶³Ü?¡5žPJ?êÈÇ.¥/@ùçb$b¿ÑB°Ž¨¥¿áÊa¸¼¿æċ_Å¿àú,hJl¿èÅ-0º²ï¿ïÿÓ?,» AGNbcu3FGL J2103.9-3546NVSS J210353-354620?ïߑi‡ö?eøKf²Ý?<~ƒƒ`è?2¨
Ê?¡?lëgžƒ?dÁ´+–6e?ïÌäü®›?}Ý­¢'¢?$QeD›"?@+HJ?xêö~œ?|ÿ%‡~ÉO?ïH%JÞîð?|3 ¢­?g`%:nÅ?U`/减?"QüÔ`Ý?yÇàNûŸ?ïç؜‰[?Q7®O†?7>e¿ì.‡?&è.ÖªöÆ?fZ«yõ?P	ôËʪ74FGL J2104.3-0212¿îý[Wêw®À>Q2ƒ
À:«§…§WÀ<` ä¶1@!ë_ð«y?ù1†U7	?ÃÉS¯-Õ?¶Îu'ãö?ó£Þ–ù¬@Ògd¾­?ïÒÀÓoS¿î,QA¼
¿›j˜ò|¿¹Ëx1¯·¿Õz«Â»üÆ¿Û쑎2]AGNbll3FGL J2104.2-0211NVSS J210421-021239?íA«êW»H?°i¦Fˆ*?Z‡×M'4?Q|–\m?µˆ"=äï?¯ÇºoCõ˜?îè)QÃ?ŸÙûW[ò?SÞm1CÀZ?_X–òNõ†? àÜsàÅÃ?Ÿ8ÚbÀ?셺ü/G¦?¢~c¶?t'öw"~?d¸°j˜n?º¨½nI"?¢A6·PÂ?ê[ï|*;È?£üôÄĂ]?orª1Ad?bMì
mã?Æ8D®KÚ?£ç»ÎC4FGL J2104.7+0108?ìªäU條À<ªà¹ÜÀ;®ìÀ<~̕ohn@Kîí3»?þ…ä*·c¯?ԉ݁%?Ìãݵ}Oâ?÷£›0r@µ
$F0f¿ï ŒÒá¹Ä?îsóãqT?Õ%çۛò¿àè`Ļܿç[gà$¿àQþÐUAGNbcuPKS B2102+009?ï·k;ÕA?|oç¿Ú?CÁ§É?@"#Kõ?€èøùe?'?{…¸'pÓ?ï§X•UY?ˆ#]¬Zó?5åì^¤'?NÈia÷ߙ?…zÊwµˆä?‡Jw¾8?îYOÃÅÝ?'8m¶¯Æë?qaVA=ò?c¨8mîs×?¨C€;›ãä?'•jaCž?ïr{2¯a?y›P¤j±•?N´êwœ.È?D™ÑIaV€?ºòVVý?yÎÞqÐ4FGL J2105.2-5143?â÷«ŸDm1ÀD¹Â.äÀ;.á"ÚîÀ<‰"'Þº@yÝîÞ¦@E¦'¶(F?ŤK¹¼Ïª?më«¿säL?ª%vkí@ô¶ùPäI¿à|¿n?x¼¿èr@úœñ¿å­A—$¿ç™¯Ôn¾¿ÚQ¯<Ü)¿âÚÒê?¬AGNbcuPMN J2105-5145?ïH+€7?˜þ'°[?NÒÁ撩Ñ?CS[¼ÔÁÿ?–ù¸?˜HjזªQ?ïskÀÒ«¥?Œ¼"­CkÝ?=ÜÍ=[Ü?RËy#µ>?'°µk?Œç	£@?î0‡ž?'¼'Ÿl®?w<Ig'×?bp`~­€û?¬ªö¾aãØ?ÉƒìÐîS?ï2ԝ9–?q:?jwÆ??€Q%D÷?4Ci%…k?Š÷HPoç?qnºïÐ4FGL J2107.6-4148¿µZ Ù€™«ÀE>$_ZÙjÀ:'
[2U¾À<|2;¼n±@N ?ûîx@Êi`êM?Å–)̓×?»¸€ºz¾?ópnAüú'?þ0«#uü¿ÏkõÇl房à/ž˜\¿äo¾Sã,¿å`ºÀZ΃¿ê²M?Mó©¿ïÿ&ñÜPÎAGNbcuPMN J2107-4145?ëÞR8g}o?²±K
˜‰N?€ãE	RÖ?{£ñçuÄ?¾ñ
T"ê0?²LuMƒbû?î=ǓŠa?¡–ïč¾?tI^SûTð?{N›p!&ñ?©¥×¼Gï:? \ö#DíU?íjõŽÛa¶?–pۑà܊?	ry"R?3X҂?°¥ó¬†7?'t8,ø3?ís#æaË]?'mã ¾dÓ?'9/wBpŸ?yzbv?°"ï!í?Ž3tY6û¢4FGL J2107.9+6006¿ä(Yã÷@ ØÀßXÀ‹À9î²-å™À;'KZqež@"eæ
æ@ß8úóPÅ?Ë$kYÀ:Ã?ÒS:»@gæ³þŸ®?ú˜€â¾{¦?çôS>kuš¿ÑDŒÂÂ#¿é´÷!¿æ_iQÓ1k¿ï÷äÞ;Š¿ìue<š»AGNbcu4C +59.33?ÒñA{p¶?ÀÀˆK r?¾ïδ×U?¶Œ Aä…?â©|q]»?ÃBI©É—?Æ*òQrއ?ÃØYÃH7|?×	 ˆnL?ÇqƒøJÖ-?ÝàæNØD£?Ǜë"@üî?Ó{ÝÁéË?ª%	ùóF?ÅMLÔ¶	?£ÁÎÃsQ?àú}ËÖG˜?«Èxîw?¼R%kHH5?–㨗>€p?Ú)½á¶û?±q…¨ê\å?ÞÁØçL6÷?¯Ÿô†'4FGL J2108.0+3655?ê጖'/ÀÍ
Œ°}À:ÊÓÎHÎÀ<&¿»lR9@ x¿úeñ?üe&*64o?Á?öût€?ÃΕ¤Âl¢@ª‹ÄÄÀ@̝–~\&?éåïé1‡b¿æóóiâr¿Úª|€Y+À¿Û
ü]^*¿×Ù#"™Þ¿ëS9bøÝAGNbll3FGL J2108.0+3654TXS 2106+367?çŽ÷,£7V?¼d‰GjÛ?™=¹©HÑÄ?§ü÷¿Ið¹?ΜlJp?ºr	)̕?â¿ÄR"-?Ƽ-Pw?n»yW©R·?yWÿ$"°w?ۅ	"«"ÿ?ƞÔÈô@?èëZ3;Å?¦å!±Í2?•¦‡Ø?Ì÷ö$Ð;?ɞá·.'?¤uNªá4?é̃Ãð¢h?žRp7N:-?'Âl¿`Å?{¼ç!!?ƕ£XQf&?žG''|[4FGL J2108.2-2454¿ïdÊÝªÀD¼j~ùÛÀ9î/²u2²À<Sîe£ÈÈ@³P–‰@_êÄ.˜š?¸œ£å"5?§¯ýˆ¬a?ê¨Ñz±w@q¢Æi}¿Ù#ñÁùµ
¿ãô~ø-£§¿å¯Z@hOö¿ép'D¿é0aœ¨¿ïÿì^ãe@AGNbcuAT20G J210812-245233?ïå&¶Ôó?j,`ÛL±?8ElF¹QE?1\[À'}ò?gá+ÀSâ?hõoù6Ç?ïŒ/!Ô÷Î?Ú¯‰m^?;136C¤?Q¹Ñ/YÖ?Œ­ñŒ?ŽÛ5N7ˆ?ï;ö÷O³º?{¢Qb"p?håç¿Pì;?Yeš²^?•ddk3?yu`|Ф?ï±v¯¥É?j¡ìpûð?XUû¿?GÕK}È>Y?€ iv*ß9?gd"{O¹4FGL J2108.3-4824?ánÉ_ŸÀE)Ëeè'À:ÈV%¦'¶À<P–ÔÃ;T@æÅÎ*ñ@B÷<@?ÉÔMI´ÔÞ?'4ëïý©?ÃÏÖ¢"@QRÔäv¿®pXœhß¿åF/ßÁœ¿è58@¹-´¿êÎô$)ªô¿æ§­ŽC$B¿ï]6=©¯AGNbcu3FGL J2107.7-4822PMN J2107-4827?ï~ Ž[ú]?Ž2õ—	D‰?f:àZ_uÍ?eVês–Õa?ŠÉ$Ri‹?ŒŽ~ÇÎG—?ïFÃQ.L?–BŽŽÍ•Û?Lúíôˆ"1?bC`ÀbIC?–?¾j›±ß?•ebÒVO?íQRÅZVB?—ùËsNä?ƒùÇ㌨?r\·ïm	?²ö0Ø»Í3?•°…f"V"?ïVpÂTkº?{""®—"?\ëTnýô?M²›îk'?"c2u+˜ç?z7½<×Ö4FGL J2108.5+1434?è¶áèV¯ÔÀ5¾p'IÀ9¿%ª´tÀ<#M"M@tN?þó'@"9¦û`?»ÿüOq ?Æ #÷V
@@ç6žË@žâ¾ü?°‰c–}Zt¿ç‡ª^7éɵ ÝD¿èûDå^³¿ïþgä맃¿ïna'·'AGNfsrqOX 110?ïÎOvÝö?ªß<àÍk?oß-±f¯?¡)ò᢫?b¨©ôX	Ù?'¹±W£"'?ql?0yÍRiõ?Rè¥ë¨¶?bo¯«ýJ?‹=/Ü5?¥¸àM?îíËØ]¯Þ?‡±_é¥O‡?~1f̝)×?t)Õ(˜­?šº+A"¹Ÿ?'ÛÙ³©_?ïIÞÐÍ.
?x]T@'?€AÁÂ
kÎ?j®Ý«Ã?FŠ
§Í?qÃ>·öþ4FGL J2108.7-0250¿îì@Q÷À?–E"}À:Id?D¹mÀ<cÿå(
e@<*žµ@z͹[ÖÀ?·˜SH|p"¿•4beÙVQ?ÞùI,™»þ@ƒàṗ?îñ/'¤ŠŽ¿ß'r¡L%¿á´M¯¶;'¿á§UCÿ3Q¿ã61µ"±«¿Û×[µ2AGNbll3FGL J2108.6-0250TXS 2106-030?îó,úé¨?" ©"Ž?dQÒ¿«iS?Yë×a?Ÿ&JՒ?"T=
*_?î¾cêe?¦ˆš§&Ko?XÀ|E?]?c~뇤˜?£SÄ/²í?¦Iàkï±?ís'¿Y€?–ÍûEeÌ?F
ohPÞ?pR¥ˆÌ?²;(¹H)à?"Pß$R'¹?ìýŒcÔZ?"«Õ£jl?†ÀaáR•È?pT`Ƶ«´?µ;¥2ÝB?'hìc7 4FGL J2108.9-6638?æUÙXvcµÀCÄÑ¢À9‹á¸À<YŒ~þä@‡Ëz½5€@ãÔk&¿‡?«£cUdá?yž	>7á'?Ωu¯¯†@38üö¶*?éÅëÒK'Ï¿áS
æû¿äÚ?çvœ?¿Ü!¾@ÂèÈ¿âÂâ2ŸE¿äÎ%\°ÚÿAGNbll3FGL J2109.1-6638PKS 2104-668?îÙ'™é˜?™¥/U$­Ü?jYÜƍ_Ÿ?a øg»e? Âo¹ø'?˜•
ˆÉ>?ï@'Þ?íš?™‡–ûl.?Wí#õuÁ€?qA2Ãé?–pÑøªðš?–¨[ow?ìJòS¦t?£,"Ÿ†.i?‹{ÈtßÜ?|õ+žæ"ö?¼mxôT0f?¢jÞVä-?ï:Ê</T?"€Ê Ü?…厗åpy?rÑ#[ª9?"…ßl‡]h?|؇ʇiÖ4FGL J2109.6+0440¿À:¡^ˆ³À;䃧 À:f̧ãß8À<-Q{×@ЕYC@ÖÎãþAº?³ˆX(¶?žÚ܍"?ßÌ¿`Ón?ÿ`™56Ä?îÂL ˜?àöÚhµÌ¿æR,¾}¿à+›>µGu¿à¢–˜]Yw¿ïüàÎï½AGNbll3FGL J2110.0+0442GALEXASC J210940.09+044000.8?ĦC?œÊ_X??zz®Er#?p'‰©»7 ?¤¨¯;X?šIÁ7lY6?îéòÒ'ú?˜~eª³‡þ?^ç/Ð(?f+.;³? išÜ¸"?—Rè§F?ìc†šÿòÑ?žh±cGõ?;±«Â‡?yõn7žë?¹<Uêñ)?šæ¼Ä
'?ëÚCÔ»?˜räBß©?—GŒYÉ?Òè¶8?»hsþCá¨?–$3¨Z4FGL J2109.8-8618?»i¡óôó¡À=.î¢
À:ˆ^iAâùÀ<pär@!™lä.é"?ûdÏÝùDû?À÷g€æ¡?¥þ®Ç(H?æÿ'ö֌?ýltóG
?ílŸWŸ¿á}Ó %¤Õ¿á•,b³®¿Øp¤ý[¿È	û÷ݝ¿ß IaûcAGNbcu3FGL J2108.6-86192MASS J21101113-8618473?î)m¼´Æ?¢Ät*(\P?`g"••C?R(,MG]%?¬b«ëebè?¢–XÀª?îÉ	(‰Ã?¡Z+»Œ|Ä?`Ä@ü;R?sj"ŠJÂã?¢c-3^)? ;ÙD›Å?í%êdÛñ?›ê­=?u˘`Ù?bœ»¸
`?µsõ¶Ð—?›DĜä†?ê
n8ùŽª?¤¡Xʔtv?ƒüüœÌ|}?v§÷^ù°	?ƖwRLý'?¤ýõ×k 4FGL J2110.2-1021c¿Ø¶¨s&=ÀA½¾ôœõoÀ:¢v0íÀ<@õ0™%@t››&Œ‡@°HàC¢?Ëç"Ï/~?Å.¾¯R¾?ð…£dôv@ZKë»ÐP?ë™H`–Üx¦ojñæ¿æÌ<6çô¿ìŸÂÞ6œ¿ïôÁ]'çü?ïÐù^#øAGNfsrq3FGL J2110.3-1013PKS 2107-105$?íÉfÝ%?®e˜>ð?uK*ÕY&?nkœñ~G?°`j)E`?­Êê'8íÑ?íåû¹£`ü?©Ïø™U²Ë?{=.PÐ?'VZYüøò?­Au5ìR?¥(Êbìÿ?ì=Kù:?œ;4tŠƒ0?"ÈýÆP®Á?'%ÊÛv÷·?¶cÖ.¢É?—ùî	X?í29þSë?˜ïIëyS?ƒhT'dR?qð҃¹•¥?´,ö4?—É)QP"V4FGL J2110.3+0808¿ "$ÐôîÀ9ëOÆðéÀ9ÌŤº_À<6ڇ s@Ò¡ÍðŽH@ÓÒåëÄ?¸r¹ÛÙZ$?²)°þe @?÷™DrØ@{Çb¦ÿ?ï1ž2°¿ä‹a'¦ãÚ¿å$†È½¯¿ânå€ÍÅÆ¿íKòa±ËÀ¿ÔOG› AGNfsrq3FGL J2110.0+0812PMN J2110+0810?ï°FÞb«7?v¡Bc]Ò?Kþ
À3ª?Ah‹Œ%%ä?'.g‹Qù?uh¥¶ñ?ïÈûyÁü?~0Úüë|?+èÁ·Y?=ÇC®Þ?zª3Øõi?}Q»Í&ً?ïO¶©rF?ƒ'þÃËu?v{!´yÄ?q"¼Ú,²û?˜—@½Ñ˜¼?}ñü'˜•?ï­bD'Xª?f›ù!?U»"ví•?CJ	µÌb?ïþP§7ï?d(	["N†4FGL J2110.3+0404¿á=$Dœ«âÀ<@vžÂÎFÀ:œiW²n}À<T§i¦@  捓&
@>:}ªOÊ?È÷·1/"?¦FŒ~Õô?á6:Ÿ8?@©m˵u˜?ïî5!õÉ¿éV­@•ql¿à֋\¿ôw¿â:s™TÐ<¿×àcØl"¿é*''¥AGNbcu1FGL J2110.6+0403NVSS J211019+040418?ìòg¨[Ç?¬+—x'?[‰e±ßV‰?N	á$à?¸_+õ¤€?¬waTþ?ïü€*[Í?–Ñ¥âuY?QÉ+ïJ%®?_¬%˜êÏ?›cÝ;¿ãÀ?–9ä×?íFåè­»û?›™j®?t#.ƒ2vú?cÑís.ì?´†Ò^ø½?šº€8ß?í_2É$°%?'Õ7me?bî°ì+Wx?SۜQû¥—?´nô/y$?"­û=µí4FGL J2112.7+0819¿á{ƒ<³jÀ:O9_JÀ9ìT3]û^À<%aþÈÈ@ 'òK—
?ü˜˜è™²?ÀüššËrÛ?Áƒœ—¥Î†@X¡ß¹8›@
,íZ`ô?±'l©¡y¿Ë¿ˆ®å±¿æi\ÜJ¿É ¹¿ú¿Ýù"ÏbÔ¿èîö«¢AGNbll3FGL J2112.7+08191RXS J211242.5+081831?ïÕʟ«æ]?fZêᐈH?H·À€û?Eu6BÓZâ?r¹1ü±Þ?d\»¶ê?Så¶Ã?ˆe±Ë"`Ô?@4CWÊ ?O\¿~­çÏ?‰Ñ§Â\Ҋ?‡Ž¡¸`7u?îÍ|JÑV?‰d¯ž!™?jGõýÉìˆ?YJΟ5T?¡ƒ¾ëvKÍ?‡ïc· ±¼?í˜ m·¡µ?ŽdԝZ#?t*êEÿ1Û?abDœö‰?±üMíâÿ;?ŽQÆæ£nÇ4FGL J2114.7+3130¿ëKˆ™c‹7À'ÄÂÖ©ÅaÀ9ïÉ¿Ò‡À<œšÕÚ@›`Ú5k@(Ç\Jƒ²?¾Œó$?¹&äàÎU?ú:bÒ]0@6~jê¿¿è÷›bFœ¿Ú¢^¤¦#¿äŽ	Bžá¿ßë‹Ô´ø›¿í.Œ¥•P_¿×®à}®¬AGNbcu3FGL J2114.7+3130B2 2112+31?è†ÞLfٓ?Á·Q–'É?'ÁèßÄx?ŒË¹§ŸŠÓ?ˌIÌ(¡$?À®÷¬ûY¾?î°ûúΡw?¨:—pZ?o6½!"Ãý?~­ãé8•?¢üԀýœL?¦RòN°;?ê>W')Þ·?§4Í!´?§ý—Ú6G?"ªËLÔ
ì?Á;ÄÊó_?¢Öl³u\p?ìÝðœ¹?–3Á'U_o?'">¬Žð?yøóŽÚú?´pšïöƒ?"s˜;Åý™4FGL J2114.8+2831?î!£ö¿èÀ+ϑ`4PÀ:-qRR³À;ØÔà—…@H'1·]@[˜fÙS?ÅóyÄ<0?¿Xòà\̊?öl¡«¶Ó@€?ƒ"´¶¿á·ü€Ä‹‹¿èú~¶¿D¿è•«}Ç«ü¿åtÞÏ-пïþÑÌæÎ?îU—¬Y¾AGNfsrqB2 2112+28B?ï÷餮m?L'9C×%?3†•.AÐÊ?3æMÎÄ)u?F–"¯*ž?GÕ}Á¬à—?ï…í½ãòô?•ô,çįã?P¤½5: ?f{ðÎñµ4?Œoøà_Û¸?"Ù@&l&Î?îf¼V ?–$þ5|•»?bœm•‰?v(X¯nx?ª í7ˆ³?"¶>rtÉ'?ïEDiQø?4kèJ9?\M¶–6œÝ?P!pÑ%¡?•'—tRW9?€‰sæÛj4FGL J2114.8+2026?îɧëZÆ9À39"úÖËSÀ;
º(…ZGÀ<zÙ@x–@ wÅ3{X@qæ¤å'7?ÍĊÉr$`?§ë#$iî?Ýð¥dSÉ@	EíãðQ?ïÿàŠï²«¿éC_›q
.¿áÅÛAÖ¿áí6ß»¿ØV}JK¿ðAGNagnTXS 2112+202?ïëî]{'¼?aü¹õ?s§éË6?{-ÄâM¤?cVE‰è	?a—M·I½?ï—Ð*oq?†úΑ£s?7]iùëÍ?N©õy?‰Q¸êT??…ùl¿ª¢?îF[g輊?•IUÛÐ@?b»"zÑ?R{r"ðÀ?ªn'@L—1?•Qa¬BL?ïtMK+T?Zœ±=?E•£Ðò7?:굨U2K?›ÄÎI|?V":å4FGL J2115.2+1218?ïhQúi#À8k•¢"À:B—Ò<èÀ<S‰®j7@ "¸ÌdÈ@B¡e?õ¹?·DʊRS࿘=~e¶"%?â5e<š»@w°˜¹ŸÉ¿Û9"5‰û¿ÙÏ~"DÎf¿æü€xá=¿ÏÔ<ãÚÛ¿èmH7§6:?ÏéÊÉàAGNbll3FGL J2115.2+1215NVSS J211522+121802?ïå]©<?a‡v*Ûð?6Fîaۇ|?. G¦ÉF%?gÙy#²Qõ?`†åæºÕ¥?ïÅ\‰É|?kÿø‡?&7™®'4á?=¡A±?|ŸþMÍip?~Ñ$ˆžŒ¡?ïÏ'XCU?…šà,V¬×?e9책-?`©ãT×?œ^Ý~ÆåP?"S"Z0ÿ?ïi#ƒa;ó?u)"UcÂ?^LÈVgsi?OgeŠWÃ?öÃr
r?tS>fýÀ¿4FGL J2115.4+2932?Öö"<vdÀ*¤$=Ìê)À89'T؟iÀ;u™ô2ld@î;'Ó+â@òŸYÌúð? ¼nþøå?»¤Ùh¼ü@Øú†C@Ѫc@l,?ïúû^Z©D¿ÞR%fÁÕù¿å7àAׁ¿ãùê<I\j¿éJߢ<€d¿î´ ~$É
AGNfsrq3FGL J2115.4+2933B2 2113+29?ï'^"2¤ó?}6\§Ó8´?Xo±÷xf?Z%(ÙÈ?.?ˆ–m=Óó?{/‰‰Ëè?ï®Kw×!¯?8Rl(¡í?Jä¡ÿ	÷?_¨%YúçI?'ÌÀ£¼?Ú¬ÑJW?îÌE:³/š?"*Îñf?‰¿+4C&?‡vêû?;?™—Ãxyº?ŠÓ!Â^Z$?×Xg;?rüÁcÈ?_¸µ$L
ã?QþUdŒƒ¥?"e3…\¯q?qMIt¬4FGL J2115.6-4938¿î¯N-4—ÀE®6Á]-À:­Y-˜¿À<œ™µHKÉ@.­f*+x?ÿPpûëžI?Æ<,9
ä?¶X|ÀÞ?ñZë­ó?÷<T "ž¿ß¶,A§j=¿çûš«'"¿Üˆ%=|7^¿Ý:ŽÜ§5d¿â\LœÄß¿è òž˜†õAGNbcuMRSS 235-024179?ï»۞?"QüÚEù?N±¥âÛ?BZ50w°?÷ž×cÇ ?""c,J÷m?î<v¸¬jÓ?§lî,z+Œ?nÈ')3Ì?z90Éê?ªL¡_?¥öÇYv?íûKBo`?–æIì6?u¯ù'"?jkКY?­™§l´&ä?Ž·ÿX–5?ëM1ÐyÀæ?¡P:ìØ°?ŠÍÄ}-YÓ?wš}qKÂ?Á\vF&Ê? æ1ÐÖZ4FGL J2115.8+6753¿ÞæY!³Ò@*	"ãÿïÀ;Dœ)¥ìÀ<"!É~c³@!m£4"‰?õÒ¼›&b?×u»Cš?ãӕsš+@ryJ@;íÞrÔ?àcƒ'«ìX¿ïÒ5A€R÷?áóRÝóe¾?ïÅèít¿ç&~"j]l¿Ýqü¼Ô‡+AGNbcuNVSS J211618+675324?ì´¤	@@?±µ&µX—?–dB-71?'®ä^?´ÁÙ%tp5?¯m;ZSß?éön¬Ý¯?Ê7$+xTi?¡Ïi¡_Ko?¶ÿáõ?ôÜô¶l?Ÿsä½-ã?ëáqä­?¦XúuÔön?—.Ž¸ìC?"Þ¡Ó_–?À¨yùOÀ?¤µ¯að'?êùZ^ym?·+vú8ìÍ?'ê›!¹O˜?—6æ°'¶?ÁÝC#ŠðY?·')ò`Z÷4FGL J2115.9-0113?ï¦Ç¢kzLÀ@'¼ÓZ…ˆÀ:M´ÒÛÇÀ<d•^¡v@Ng¹L½H?ÿùäwä=,?‡o vØy?ÀOâ€é'?û°ÔéÑÀR@šsPڎ¿ç*SÆP±É¿Ý‰å£©¿àâçÁDÙN¿ÜxwÀ«×4¿ïŒ~"ƒÕã?é³>¡%AGNbllNVSS J211603-010828?ïjÞ´4ê?z3Výs?mÿÀÙéB?mØ~"‡E?Èˆ|K!?ŠÜ;pk~"?ï6òáÏ?›:µzÌ?`¥Üd?nªpfí2?ä}òWD(?˜±ø9ڞ?ì÷4uç'?žNè'zÚ?œ‡l"3á?'AN‹/¿»?±$2s6…?"×£±Ê!?î±4¦‰?ˆ¸¤?wM§±*•?jp~²XÝP? ë7¿y"¢?…x¼"½É4FGL J2116.2+3339¿Ò~5_ª­À%MOçžàÀ82LOcëbÀ;[í¤³©@¡Üí+g?ûòˆ-`‹[?¡Sʂo±i?¹.nRn÷@]Û	íÀ@¸Ü&$?æÇ·ÿá!C¿Ò½·†ªØ¿Ù"¾h…û¿ÙšÛ
,c¿âQßƤ•¿à`䡪µ AGNbll3FGL J2116.1+3339B2 2114+33?ï¦9<aXœ?znòŸÜ?C	L(Ê E?B+Z¹*zë?…A%6Õ?yƒ+÷d0™?ïNÁvÜ}Ù?¡šá°Óò¿?YÓjíã(D?y¶NMKª?"Ššu'??¡	¥ZRr?îœ|.)ç'?"÷
×ã&C?†¸.?ƒâ'¶
9 ? ²|o]»"?Š¿‡`»?îâ¢iÙ?•6ô½hÉZ?qcÁÛ0?_uÊóF˜[?¬egŠyV?•ًœ–V4FGL J2116.3+1015¿ÏÌIôYoÀ9Ý˼+"ÙÀ:û,¨Õv¿À<e¯¶;Ð@ÇXÛch…?ðx
Oš?Ü¥0úØ#?ïÿì´É È@®-±éò@ƽñÿÁ·ù«
	¿ê
aw¤Q¿Õ©úºÆ»¿ëtÙé¿ïôL¾´ ?àV"Zî¹AGNbcu4C +10.65?ì´QƒÕ?¹J3ter?{¹'ÿ§G-?ƒAØ)raö?¾>ÅCí,ç?¸×ƒìVÀb?ë±cêÏR?ÄM-Zëk%?¢¨É‡©8¨?¸ØKæYB?¹ {å°Ï<?¼OfÚèí?ç¸ßÑ`àY?«á8tá\Û?´ÙÐ9Œ,?™w>I¤Ec?Ư˜¶h—?¨ã_úb?å-u(KÕ?Å·c1Ã?zA'}eA?{×`JU‡æ?Վ w¹Óé?ÅÌ<µU;v4FGL J2117.4+6159c?ïóWQºK°@!µo—g2À:²aç|À;ÔUÓq+¼@)Ñ,­Ýô@Ò¦-?Õɞoc?èÀ‰þ#r@
fr$àŠ@¼]Sm:k?ïþnÀ}>¿ÚkJw—¿ç<"Åý¦¿î-ë•å¯ó¿Ô}¢'¡Zƒ¿ï¡kTâ°dAGNbcuNVSS J211613+615920 ?῍ŒOJÊ?ÌóVÙ	å?»Á8Â?¹&»[†?Ր–ÃZ9ê?ÉÛϵ&Õ?Òõ–çãv?Ì¥ý,8?Ì1Þ<"ó?ÈPZâ…N?ßÍaùÚ?˦6kGq?ÝGÛA9?­òÍ)_?Èÿý¤‰?©2ç¥Øƒ?Ö8"îz;?«+:Sܽ?ÑÀLŠU?°{(ó%‹?Ë©b¶™J‡?»«é(ìh?àŠ›ò3h4?¸
~".á©4FGL J2117.8-1521¿îE;¯"¾ÐÀCp'IüÀ;Çwù5áÀ<hP?³t6@ÌYjÕa@ÏãzŽ;˜?Ñøòû4¿$?¥OiÒ~?̧Àä6Jë?û`¤$âãe¿Öa·˜ˆ¿Ýþ‰Î´¿à¶+ —ºœ¿çRÜ{–yT¿ïüt$•
¿?ï¶ý!ÿ.IAGNbcuTXS 2115-155?ï?aqw?"	g?0™B?P‡Ì–ãiH?Iút¼(ˆ<?›ï¢Šcšz?'Òʚ4"É?îTA?Ê1m?¦¨¸>Ji)?q‡?goœÿ?[ì?¨‹nõt?¤ÌµL•Uq?ìòHVŸpŠ?˜§S]"¬?•8|Jf…(?…¼~ÞÃ*®?³ž8jÚg?"¸NH…Ê?쩑ŒT?Ÿ­Õh*Ã?sV,è¿Âe?iĬêO"?¹~Ñ9cS?žub¯¨34FGL J2117.8-3243?ïÂHGu.ÀEïÚQÎÀ:z[ôœïÀ<M\ú¬Ùè@ ZÛ¯"«ï@eÏ?mÔ?½h"£¾5°¿šÀ>ÁS>c?ßX´Ae¥÷@ËÃw?ë€FvÜÖ/¿àÀÁü28¿äVóAUµ¿¿ät9Ûr­¿Íy¨7—¿ãý먰AGNbll3FGL J2118.0-3241NVSS J211754-324326?ï.éû·&?'~=íy5Ÿ?`¦í›Ð?V.š/¡z£?˜
þÜ«gÛ?'ÎqP[Îd?ï?ÂL)ÇÚ?'Hœú»ü?QRf)©³c?\ùó}à%?–ò,iv?'W$Ä¥aƒ?íMͤÔ?–Åæµ^˜?~mµ%p?jÚ»7J'd?³°'
"?•¢È°Q?Í?ìÙ}Ǿi×?™Ý.dB2e?vgΛÃß?lB¾&:ŒÙ?·Í"Ø\%?šBax˜84FGL J2118.0+0019¿Ä\ñ— \[À?è">À:¥6nQsÀ<Wæ¯Ìâ@ø5˜hA2@ø'œ&;Ô?ÝíM
tÎ?ÚDôPÊ?ü@ÇÀôQv@SÐ|"`¿ßc[+J1¿ã­g¬·"¿æ*MçŸð¿ívjàžÏ¿è¦ÞHJG¿Àzz(ÓAGNfsrq3FGL J2118.4+0013PMN J2118+0013?íˆ9†Ü¿
?³N‡d½ñ?s5Ÿ¿Iš?‰ŽKÆä×?²ŠÙÍ%n
?²ÍSeä$?îÒÅîÝ~¥?¤‰:}ɘ'?hnÓy"€?{{*Ì+Ù?¡L¿äð}K?¢º&.áuÑ?ìÉ¿ù&¼?ŸZ:j/?•Y*' Äƒ?…VžCHÃ?´[µ–'8þ?š?GÆiã?ïd^dõ4?{ô;ÐYÒ?=A†K].¥?7ςÜÃ?'ÿ&:3äõ?{¯`(BíÁ4FGL J2118.2+5752¿ïŸNPts@¹p]`-gÀ9Á;ϹçÀ;™j×o@àçñìA@	'C‰ÂŒ?Â>ˆ;xQ ?Ä}þ&×Z@TŸCý…Ò@˜öChµv?ï"]9–û¿çÖ´âË;Ó¿çtŸºšñ¿ç8×L''¿è©ç$f疿ï¾àÅýüAGNbcu3FGL J2118.3+575187GB 2116+5739?íÊLºŽÁj?§éÆ|z Ð?{½70€V?z¾'#\†?¯ãq¹M?¦ÃS¹—'¼?æߑW-öÛ?ÆflMG¡?‹Yü%?Ÿöñ!¦m€?Ñhҁú"?ņã¬Ï§?ë^ЖÍ?§›uüiË?"îç|dR?†Zá€+?Á%±•1!E?¤24RbÙN?é>»õ¨
?¤hÕ
¥r ?'Ne9½;>?yËàD¥}¼?È»C''àe?¤éE¢A4FGL J2118.8-0723c?ï¾D¤سÀBhß½jYÀ:ª(҇ ñÀ<,=]…@öE(þüË@8\gßã?ÍuÙ`ƒùI?Áޅ†è!?택Âô@¢ašú—¶¿æpoiDg8¿ån8¿,Ñ¿èëõÈ|Ü¿í†Ëá•[Ç¿îèïwòå¿ïÿüoQÇsAGNnlsy1TXS 2116-077 ?ïâj,Cy?p­TJ5/?BXYc$µª?Aôþ˜(?hÜzóZy?o…ඇ,'?îýt¿g'?¡ö,óÀ&?agþa`†?uÄëì7ç?ž-'ˆFãŒ?ŸôJ=…?îõßB0?"Lx Âƒá?~zGVn?t>²fúR†?ªÑY!*R?'¢4WÏã?ï2ߟ¸<ð?GÙ=έ_?c'üÆϺx?SiWx'$º?—?pj¡?€æ	1Ìm4FGL J2119.0-3317?äç SæÀFbMÒñªÀ;Ykã}é:À=!Iâ¢!@ÉH±Æj@ÃRë__?Õ.³R)˜?ïÔËi~K@ëÿÛk@ŸÖ
=UK¿î~ߧz®¿ØÌü½«FÀ?Û¤]Aúv¿æ¤Dî¿î1Ū™œ¿ïöF"¤ÐAGNbcu3FGL J2119.2-3313PMN J2118-3316?ÞŠ8W?Ç;ÊU\ù0?ϋÔc¬i?ÃM|–é?Ò3è]»v?Å.y¦'I?ß*—Ñ"b0?Ð0vLIS?Ó­ó³2Í?͵"¡(¿?ÊOÌupÖ?ÀŽ
̆k?â¯î£~™e?·>BEd?͛4g"Ú?³Òëë?Ç¥
âÀL?¨7§}+¥?ácâ«Ê?¿./ͤx'?֏çköòN?Àí¬º›¦?½
C?nØy?°e‰¯ü;4FGL J2119.4+4652c¿Ò lȑdþ¿þ©Ü¨#$À;4ÒÆÒíÀ<¹?QN§@!~';ýP?ýBL
šµ?ÙzGĺ¯"?î£bۗjë@	÷ÿ=ba?óá–óÌëÖ¿ïøgàŽö}¿êæe$G?îÃ߈'3š?ÕW³%óà¿àb¥ç…µ·¿ïÿÿÊPËAGNbcuNVSS J211922+465026 ?äBæël!2?Çc4±R?'ç.¦'Oü?•á´
˜?ÖK¿>¾¨œ?ÇM6˜p?¹Åì
iï?Á<£@¨j?½6 Z¼?Âìú{¼oh?é nqÚÛA?ÆÒÌ9øÅ?æÖáTÂðo?«ä˜-ş?­Pøà©Þ?•RºÐ1à?ÍPu.¼Î?©;ª%ò´K?ψIO|[Ü?¼¹[|'Þ	?ӟëqþM?È%ßè ?ܜÉlÏÓÅ?Å{äþ+R4FGL J2119.6-1105¿ç¢·æ
áÀBñŒ~($À:oÍuhÀ<KÛ$~dŠ@9"v¢s³@þZäR%?»§!	K>?³Ó}kÃl?õN¨‰÷e'@édZ&?ïìpk¢æI¿çóZ4ÿ¼
¿á¶ôžM›¿ä~q f¿ç™ÌYàF&¿ïïÀý¶¤—AGNfsrqPKS 2116-11?ïßÁ³.+"?cw¬%(ý?-ÆÑ°'"7?(zB,¥Ú=?na߶Òc…?c
…~Ø։?ïÂ5² Ž˜?'ªžˆœøñ?(?'3_Ú?Ax—éGª?~#*fÉ\?'?Þ?ÌÕ°?ïbÔ;?'¥Å[eh
?pùUUŸG·?kcôI.'—?™gÎ?õ£U㆜?ïÛHÐG£ý?[P{i…«?4/²¥\_?#¡Ûñë~Ö?q¦Qªþ?ZnÊâsQD4FGL J2120.6-1254?í'*)Á'ÀCnş±áÀ:hß۝J(À<d×ؙŠ@ÁÊÍC?E@}!xö‹ã?ÀÍßÇPa?®Â_œ®Þ?ìܙÿ&ó@€×€ÚÜ¿åîO¾Úé¿ÑŽ)ùΎ¿çñÝþMx¿áõ!HÏþ¿êŸåãõ~¿ÓUžã/»AGNbcu3FGL J2120.4-1256NVSS J212035-125443?ïÇßQΓÐ?pi÷Ñ´U¸?J¿_.ÊÄ?A	£ORV?x¸k2Ü¿,?nGŽ¤f~?ï¹åXìAÆ?'À]œ%*?"³±A3?7ˆD0Ž'?;Úÿê›?']ûžZ?ïÕ%¼F?…ìƒk®´?uCUd$"?q
6jXô?š4…ïn@?ì_O"?Kwè?cïz‰«®t?NŒ»ýx?;Ÿíëî?}ç²æŒ¨?c=Dÿ¹@4FGL J2120.6-6114?ëÄ»m¡:šÀDžî|IýzÀ;!—rwíÀ<¸£ûó+@OYýÍK@/ªJè\?Ð/níôdÁ?ȑòƱ¿?ölaR*o@œ7^+œ?î]ÝÙ¥¿å‰ÚÔ¯¿ã¡Œý©äj¿äsƒðºèŸ¿ä¼27Š±¿ïþ N¿€´AGNfsrqPMN J2121-6111?ï»WÃÕ9o?vWÙ?z-ü?R¹‰}x…ó?J•ˆÕêО?}¥»¶'K?u%Ú»XP?ï/6JÆf?–Ïs°%€?PÝÏB¼?_A¦90©?™<F6/!?•Ûâ¿oéc?îyˆ:?èÅ?Œ˜?Ûçƒ ?xã°ôà?lÌh‹0†é?¥e?‹U"?‰0¢N¿÷f?ï5ЫîÅ>?{nü·ª?`xr€r‰?O"|8.¹$?—6ړ×J
?zªáT¡Õî4FGL J2120.7+4428?î_ff€+xÀ<AÏ®)À:?±~'­À;¨iTWp)@æµ+E~@Q*Dw(V?ÇI/ôºQ ?¡M¾ú§%ž?ÚiœÁAS@d‰ÉAþ?ïþj~£ôç¿á+"}¨¢K¿ëáxU|¿á2Åð9¹_¿æyÂr«Ä¿ïÿîbHÊtAGNbcuB3 2118+443?éhñG]à?½m¥£¾)?tø߇×;?q"Hƒíü?ÉR•>ªqÆ?½#~Ê!ÎÝ?áܜâ¸ö?Æ|ò»‰PÎ?eyéòD6r?xü×ùþ·¡?ÜÒf«i¦?Æb\X¾ƒ?ᮅM]ø?±*$¥—´¹?¨WšÙ?'"$!ø}?٘¢âð?°%–yÔk`?ê_cwÚºŸ?¥+XûE%Á?‰Ú»ûŒjò?t[Ã×G?ÄäÆ`ÜNÔ?¤Š	÷4FGL J2121.0+1901?ï´YIiÎÀ5>
 r~À8Šr©jÇõÀ;£ÊÖR‡Œ@¤Î(š@>Õ®Þ]?¢^/š;?­c|ö÷@ÞZ"Ê@
yñßÖ¿À?³mÖVοá÷u¢™r'¿ã‰-°ê¿á|¾ß¤@¿æóBýօ¿ëM³"íbAGNfsrq3FGL J2121.0+1901OX 131?ï°:pÝ?{x(àkpŒ?BLô¶§¿1?>(øõG ?'Ì"}P¢?z‹È~ƒcÐ?ïIáªÿ¤?–åêT´5?gYT&)?z~ž»]ù?"Ø 8ç®?";S²ÙfP?îÎÓEüÿÞ?'Ý "Æ#ï?~;Ö-'Â?~(6A1d?ž–¡´ÿSµ?.:'«Ýø?î<'PTå•?Ž#3Œ­þ™?Ž}ðÆ¿®ã?{@	]9@]?¤—nɺâ?ˆº!ݬ—4FGL J2123.6+0535?¿7|Õ#ðÀ>µÜyÀ9é't1*DÀ<6¶NÜ&@½'ãɾz@
b*Vì?´+®À®l¡?"plN²À‡?àFǨ ž@
ònòÑï? œƒ¿â¨b8Yc¿èž»ýq°G¿â´ˆ"MÝ®¿áØ­«ŸU›¿ïÿânÁŒAGNfsrq3FGL J2123.6+0533OX 036?ïÁäþ—Ô³?" 5'°?C¸2"q½Q?GQZDQ
?|–zoÇn0?'bhÿRJi?晴ó X?…6%Ljù?2àÜñeŽ?Lò[#‰?…D<P^ӄ?"•"è§N?ï2 bÿgé?~t()ÇÏ?i'wCdº?Xêüd°'?–‹¤·²–%?{œ"×b¯?ï†l'Ÿ¨Y?p.!"–©,?c.ÃÙ%Ì°?OXbŒÑl?‰™.aÌv\?lú4ä›ï'4FGL J2123.8-3148?Æ»ú.QCŒÀFæÄŗNÀ:µkÞuk½À<KŠ·~‡@Ï¡ê ó*@™cˆÕý?Ô]•\s"?à¿-§Ø÷}@0[b&eÅ@^lg1g¿æ"íٌÏ?ïçô÷í¿ë/•XÆ¿ç2UB&Á
¿ïîû.	(¿ìZVÆy÷AGNbcuPMN J2123-3155?í5/ìRe%?­œÁxO'ý?'Â4Ö¼ØJ?'ò'ËÈ?±¥óg½ Ë?«5ë?ì~‰šýâÍ?·2½-pX…?˜ÜÂÑk[?¤É<Îé6=?µÔ's¶Ö?°Ë]Wþë?è<äL±3?¬¯GÖýH?´'¯ŽZ͘?š ̶ëK?ÄÃ(h?¦5+à†¨?ì¯t­À?›BC¸Ö?œ6Qä8_?Žj[\¹?³y³Sì?–$훃T<4FGL J2126.1-3922¿ïç†p‹ÈÀFþ"ž­Õ'À:µ~Ư|ZÀ<"ú~Ù@ÕôÜ5uƒ@™ñ®-¥?¼A<á1ޟ¿£²€f­?çÀŒ¢8G@!ýŽ?ïý¸ýâïN¿ØL9)y¿¿çê¹aµý}¿áY3BL«ª¿ãùïzv¾£¿Ò<ªÏ'AGNbll3FGL J2126.5-3926PMN J2126-3921?ïÆ¢Ú36?"$¢HF.?Q$FfIÎÙ?G¥­P]?ŠiÎ|©ø"?ƒK-G<i?ïY?D_jÞ?Ž÷…FEé‹?HÊn\ðC'?Yæd·JØ?"Ä+"9?¿'3ïá?îaà9aÌÜ?Œñ‹ÐÈ?tH^1ò?bk‡ýŠ³?§Xè¾ô?‹SäQ<Ç®?îäÉ2²?'zׂÞÊ?fÙkyBï‹?VpdŽ? EÙ'h¥î?+gîDÏ4FGL J2126.3-4605¿ÄSš7_xóÀFÏG0@9¬À9kæ'øÀ<5/Ùâ_@\XúÂÿD@Aà?pXX?¦ó5—;›b?¥P(as'?õõ+á/Za@Àw¥("¿ÍßÈýà@¿ä/D%ɾ%¿èèSpÀ\|¿ãOCÕAæT¿ë`›KJ.¿ïúÕô"»3AGNFSRQ3FGL J2126.5-4605PKS 2123-463?ïðQNåò?T´íL'?3¡~°Cñf?(
õP½·?Zu¶#É?Sa÷2È0²?ïÖ
¨(mJ?{0zÁ¹¸™?&`:‰®|Ñ?C«˜Rù¡?tF*{ç™?z[±É¦8?ï=D¹ga?Í28ýôö?jüo—hÁ?]Ø@ô ³d?"÷ï5æL?€eIú
Š?ïþ³Û?#Røû
ы?ÄKŒ€?!‹@µ'?*n+¾j?!3:o5No4FGL J2126.5+1842?摩ڞ5yÀ6m»{k±)À:ÏáÕr¼À<wª¥æ¯@ 4‡†Êµ@ÛÄÒ,ˆ?Á"AÞÇ¡¿¢|ÉCI?äMÝ|è‰@aŠžÿßõ¿ëä¡Ý4ú?ïÿÁeÖt¿êÁj=¶nç¿ÉŁÿÉú5¿á*«ýI¿àaO`eprAGNbcu87GB 212407.5+182753?ïÇ~ŠúÀ\?ud+Øè¬?DáNÅ-÷?@'Á|}?y¤©ú1T?tˆp—&<´?ïÀ
q濏?»-*¾Ò?2Qó¶µTÈ?GŠ'Š-¸½?~Õ§Ñ4ã?99>"ç?îµÍøIÙ?'ÑÃCŠ¶?qÔY·ß/?a±NAQ®¸?¬:é˜&?';øÑ5'Þ?ïO¨È¸Èø?|	XÈ¢€Ç?h9'wOÇ?Y"ôÏ×?"´ºw?z8¨<ÕeÅ4FGL J2127.6-5959¿À¡ÚSŒßÀE=¿H˒À;X?½…1-À<Üdçá%I@ š-hC
l?üuãTΎ?Ë:'C:è?ÃÃú€º$ª?÷ځNš@""¯ ê?ïîy$¯ò¿í:䜸2?ސ'¡»ý¿àʐ¢Oοåñ6;%¿Ñ²'¤\ìAGNbcu3FGL J2127.5-6001NGC 7059?îÏh¬>÷?³ëDk§?ˆG¸:ðG?³ïæ|ßÞ?™ï[ §Õ?¶»Úé?îÿv2FD?–'ËØXÑ?XUp+çC´?dFU"6š-?ž‹â´}ã`?•n#—}?íƀDý>:?'môY$ˆÍ?q[¸þ䦱?^Ö¶Ede?°¶BH'þ?Á8¤)ì¶?íµÌD?"þÚëášô?nˆî
™ƒ?c¾x'Ë
¹?±c*/^½±?" ",D4FGL J2127.7+3612¿¹AlÀ%ùÁø]tÀ9Mo«‰†&À;ËüÞ1@Ês×K?üþ_·¼^?²a>‰R¥?ÀN®ä¯l•@¨!ò™0@1<ëج¿ÎÍÅÆ[¿Ùú$‰LD|¿Ø~¤`GŽ¿ßŽ?ÒþÀ¿Þ4"ý#Ö¿ëá& þ'ÃAGNbll3FGL J2127.7+3612B2 2125+35?ïiÊ]b–?‰ŠÕd½­J?XÖ´Žä}Y?R¿‰1¼›?'9I
Ñ¥Q?ˆ£säj¸?ïA‹'š(?–M=Ög?GD´½";?mN™Á4Ó?—
ˆéÃîs?œ‰üè왪?î]ŠžF`?Ž«â¦0'?|Dè5CTp?tîú…bvå?£¡ŠOs/_?ŠhypÀET?î.Š8ž3?ŒªtWö?f:•Oý?QbY¶ؘ?«³¶«•çÃ?‹¡â
 ¸Ê4FGL J2130.2-7320?±ÕÖ՜ü'ÀBmß 'áÀ;JòÌ:֖À<Äô,'@É{ôíþ ?ý=¨!ò™?ÒáÍdø'D?Ԋ\¥Gw¹?ø*²ái<@8ô‹(?î˜32\sž¿íè†1		?²|Ç£m-¿ækµÆ 
b¿é/ôq¬¿¼%p§ÝÕAGNbllPMN J2130-7325?íÁÑbU?±òtËGCó?zeRî'E?r¸èÑÚå?¶I¤Â‹É?±~äŸJv·?î‡
åüô¬?¥v˜™("?ied´iu?v¾%þ'9I?¥øûT辡?¤3Q³c?ëèÖMàR?¢kB¬¢'Ý?šCÒZ"Jª?ˆ…«.í I?º(Xúr'¼? ÊU0]v?íÓ>l¸Yc?'wø_è"?j%OÀ%Ì?^"Y·—??°"â<±?ýÏb_Ïü4FGL J2130.4-4241?ï(·ëPÀGUž™ À:•êњ'çÀ<t&"»@G6¢0—@Ð#éê?Æ?a>ß8à?›ÕW	ý?ø§°³'@Ù{´Qy¿éæÍÿÒ³—¿Ö"š.¿çå¢'<¿ã8?ân¿ïû›÷Ì«¿ï=I6ª·AGNbcu3FGL J2130.4-4237SUMSS J213017-424319?ïôöåõéó?X±4L»{m?(b•®'×}?(´ÝFŠ›?Sá^Y½¾?W.Ë|€?ïØ듔',?yÕå0«?!S7eA'?=/«›Ï)?sÜÀn?xߜËb•‡?îÝðÁæ&q?‡2wM?wâ^}>¡V?o™'Åɒ?žIP#뉣?"0ñw¦À?ïø"ÇH~?=¨ãm1Ý,?ØàU‹Á«?i#'²ò?Mø݅KP?<Ť:x
4FGL J2130.8-6623?ïü‰•ŒæûÀD È`VíÀ:@.A[êâÀ<Äa¢—o@1O¥"´Z?üØ´|sîå?À'ý]¹C®?ähY …F%@ }(®tòñ@ÿ9Cm"¿é Û!¤??êìȀ6ò¿Ò//bÄw¿é.äïÙA¿ín—ø¯©¦¿ïýÑò¦{)AGNbcu3FGL J2131.1-6625SUMSS J213038-662356?§sÓê­R?©EïÎ~?íìd…ø÷Š?°;\"*
ô?"k™´??›×AOG-?°×¸%ĉ«?²Yð
§?êÕYK»ßÉ?¾êüøt?¸}}|\x
?³œ`Ýcn?± ÷¡Íh0?›Ý{¥Z	?ê-‰kÄ5é?¦©V	¾'K?½r½èŠ? bdo
	?Ë#hi‹FN?±¢
#b?æ%E'$?·;¥ž¡¢J?¸]jC?¤¾µBÀ|4FGL J2131.0-2746?ÚlEØD$ÀFì×à&EåÀ9‹‡T¸À;ìh?"zN@3úÑíÈñ?ùóúˆÇº>?²¼;7ó?¿	Hþ÷l^@+ý´Ì%@
§&5ô®"?ï'v Ùó?ÁDµüü•g¿ÉΆö©À¿ÜZŽâ™¿ØÇÓ~AÏX¿ãcs¢¡AGNbll3FGL J2130.8-2745RBS 1751?ï´F	o?w˜ÝWem?`Îí7
êÆ?Z"Êù,
?}u"¬²ù?tXqk''?ïd¶töa?"Òä/ün?J#Óí9ü€?Xâ¤Ö22Q?'«J'÷cö?"uuíÈÖ¸?îÆ FƒS?ŒíæÆ?z"°ì`?vÜqµ	NJ? MevUçÍ?‡'lûë?í{"Ô"?™©9®º?q¼s"c?b/P4PÜB?³`:.AH?™aa>Õo´4FGL J2131.5-0916?ïэ¾fyÿÀCÖ@|ÇÑ»À9¥
œ;5À<%Åo@	_	ç?ÿÃnÙј?°gÆä*Œ?fœÏŸ‰'?¹ìÒў˜²@
-:×ÂI;?ïsÿi­¿ßD¦âÔ¿ãÿ•g0¿ÚE¿'Q¦¼¿á•Ÿ¤u•®¿ÇôwáùþAGNbll3FGL J2131.5-0915RBS 1752?ïîΝ-@Ç?YŒv!"	%?&"vç2l?±_OW?_žvȘ1z?X"艵w?ï¿ÁO?ƒ²ÎŸ"ª?&Ö´L›w?:¥†Ž\î?Ài¶;Ò?'Šcz¶C?ï.Š8Zr?~E¥ÝNc(?còôܓ{²?Pv†õûé
?—°^]bB=?}P&zÓ5?ï—(Âý~j?mº€>xç?T§yZà4?Ajƒr?‡ àD^Í?lÊ)½64FGL J2131.7-2515¿€ÏQ-çfÀF»F^‰"SÀ:YìÝ
Œ°À<ZSÆP±É@ nYÎÓb=?ûÈF¥Ö¾¾?À¸ô'ڏƒ?¿×´ÝAäý@ÅzxQJ@iÂß84O¿ïŽI9.õ·?ê)¯[¢¾¿ÙÁa3Ϳע."'AÜ¿àÿŸY¿ÕŸç't1AGNbll3FGL J2131.8-2516RBS 1755?S³H·?º†Ý×3?Y"‡Ü?VWŽ±›õ?‹-|áó?€"ÐÝäm5?ïTŠ½_š{?"IÁÍ֟¨?PqMsÐî?]ì9™ö?"má?5sš?'>xûë·¹?íÔ?™TBA?'¶B•&ù?z7Ë텶Ú?fÏ°!öp¨?¯uí$ü?eª/Š{"?íÐkÔzG?‰È³³²`Ì?{/ýÏbɂ?f`͋}€¸?¯"Bþo55?ˆÁËðZRÄ4FGL J2132.0-5418¿ëp´7¡úÀFliƒQX¸À:	²Œ¯¦KÀ<jńÙîô@Mä@Ü¿@G?Y²#?¸y€Ÿwª?³ƒS‡ªó?ø9ߊ>²Ã@ó–ßU§?î+|…Œœ[¿áEäEVJ¿ä^_[Û¿æIøÜö¼¿èñÒÀ¬­ó¿á_L@ËLDAGNbcu3FGL J2132.4-5420PMN J2132-5420?ïL\O•?‹üj)äºi?YaK\Þ?S8sáÛFÜ?"éÀ?q?‹~"qi5?Ÿ—qP?‡XžoÌõ?:
=´å)?M/>§Ó¨?‡Æ,|P?†©=څ§?ï%buÆÇ¢?~DìVߕf?l.Nžý?`ZHÜyŠ?—ÍðÃ}8?{F?̺j°?ﯦ€¶P¼?h·-‡,¼?ZšðÁà?Gtð"Ð1Ý?€ÄltS°H?f"E=škû4FGL J2133.0+2610?ÁA¹DõÀ2q»à~íÀ:×Üßi‡ƒÀ<?‰›ár@ù¨çj\ë@¯ŠÄê€<?˯æ8óg?Ör$u*Nˆ@ýæJLT@´²@¦(?Ñ
8þyB6¿â¨˜é_¿çMFkE¿äã¼gú»¿ïþ€¢§µ¿±Y¯ô¤ØAGNbcu3FGL J2131.5+2605NVSS J213252+261143?ëÌõE'¹?²üÞ£Z‹?²Ë¯Aˆ?®ËëÝ9?­™MkÀ¡Z?¡ÛóÛÓK?éGÆZK<?ë\Ýp?¶ëRVñ™?ºi܊Çå?¾Üw´ˆ?¶ò܏°ø¤?缘žz…?«ƒXueP?·	gb€8ÿ?œT%$DüW?ňéÔÕÏ?¤¤>ßËÔï?ßn±LiA?ª0\U–[A?ÜÃ0ƕ3?¦•ÔWÑVµ?ÖÂí€L$?­Ÿ6"J¤4FGL J2133.1+2529c?⸷äÞ;ŠÀ2óNe¾ ºÀ:«ï}Ѽ÷À<j"l
ë@ ¬³Ho-?þȼg#ûˆ?Å'Pǘ°?¤Pl ‡‡?ã>Ÿ&Kn@û©Ã2o>?ïúޝڛí¿×Ô¿?E-¿à£^Caÿ¿ÎR$zˆ²A¿æ»Ê`áÂ'¿ÒƒSœŠ9ÕAGNbll3FGL J2133.3+253387GB 213100.1+251534 ?ïe.UÊøà?ŠU«·7º?AýAþp6?6¸³1»q?'ÊK6­cà?‰¿ëú{Ü?Fbã|?ˆãz‰-<¨?='s¹qñ«?Pžºò™TN?‰¦"É{'B?ˆ–—µGÜ?î
&¡«	÷?"I¹Ç™º?p+À—¢f|?\"×¹¬;"?­XÒ[Ò?'«+ײ²?îI°u$Â.?ˆ© (óG'?sCôãZž?`¾ƒÊR?¨ü˜Oq·?ˆ²—BèõD4FGL J2133.6+1439?Ïë$¾GÆ5À:d6†¤ÊOÀ:½|·¸À<" ()ö@@Ã]NÞ@ךCÅ
?Æü7ž}¿®$=®X»?äµÎMÖL¨@c']çç°¿âøâÕLοë]
Œ°}¿å'z¡0ç©¿æ9Mß0ýy¿ïæ¸f
{¿ïÿò> wAGNbcuMG1 J213339+1443?ïЦšÅ•}?¥$\no`?m/.×7Ç­?ž+õ™¤J?b*6c2º«?ˆÿå**U—?ï~[.žw7?0‰@zXÓ?Czô<Æà†?WáðsLÃB?1…•Ä(?‹Ý‹Æ$Y!?‹Bú)?Žˆ«0D÷?p÷H<?fŽ^üÚÊ?¡ýöôçUÞ?ŒšÒ2uà?ïOÍï ¾q?zșæ?YLeŠH®Â?Mz—À?"q{³C¦Ñ?zŠø&Úú4FGL J2133.9+6646¿¯ïg_g¿@%ù
{é…jÀ9Wòw@ÝÀ;òd\ êÇ@åÄ[º@èà(Ê$?´"54Y©?µ@b›«—ž@
Ú\ˆ–@½"NXӁ¿â<kU¹où¿Ñ´ådô y¿ån oQ¿Ö'°œ?':¿äé2(q8R¿åFÆÞvB|AGNbll3FGL J2133.8+6648NVSS J213349+664706?ï­A¬AêV?¤W켦~?Q(‡)ʛ¶?€HçÏ/µ¯?'Š"
L ? Mq*Œ€¦?ïqqsÖk?"*Lÿ3?RPØ㼬8?b§T±ìÎw?¬Ã÷§Ø?"
õߢ¸ç?î°'­ÐÌq?‹ætŒf'Z?râœL'ÆG?e'K°f?¢¡1™bà=?‰ÀA1œ´?îȾ—)Ž?'ûŠ˜O?wUÂΛ?b9õ+Tf¯? ‰^M³¤?ô´X}õÉ4FGL J2134.2-0154¿àÛy"À†ÀBDzd×ñÀ9àR»Ž·À<I—"Ç@Ò¤e¥vG@DfBT?ªýd©g?«èž ¥¸@=ÙÂ~•1@‹–'(6*¿ÖóünñO¿ãaþ»Ý;¿äîvjÀh:¿â#•›Þx¿è • ãû=¿âᙹzAGNbll3FGL J2134.1-0152PKS 2131-021?ïÁÀdðŠÿ?vvqë?=ö[z7j?9k×£ô?}@gÐ}?uB(·'ë¼?ï´Òï‹J?ƒÑ¶(LŒ€?7mwW!£ï?Tž•Çgdv?'Ø~$ ¡?''h·5m€?ï8E»òß?|¾Ç`t?h}×BÔ?Y7VÇ¥?•ús¸Æ»Û?zrN®Çx‹?ïÖº	1?`©ÀCü‰Ô?JD6mš€t?9£Q?q¨œ-´&º?^E-W‰g4FGL J2134.3-6511?ؤƒ6D¤dÀDc¡À:Ç+×_gÀ<aýõ}Æ@Zt¥™W@Cá8j«?Ðe¦Ñ?•ÿ¥DÑó?·™¿¯,þ¼@ª7îý`¿ìÒÿõ5¿åk›#ÝTÚ¿àm>K?D¿åNìóà¿å°¨t'ð	¿ïîW–¿Ê†AGNbcu2FGL J2134.5-6513PKS 2130-654?ï`×°Ã͉?JTü©?F±b³ž?@ÜQ7ɀ?"/~ÑéZE?Œ½ú[Î>?g<°?‰gHl<…‰?;ã*¨ýx(?L…ØRó¢?@èè4?ˆ£¼«ÔË?î%ÂƤ@…?'–v˜Ç?w§ñMSh(?qS§xڎ
?ª®ÕlŠ¤?«¤›#–/?ï!}ˆ?'i¾MŽ?L›¶×,??Ý´•GV?šëvg÷£X?'z3Þ‰4FGL J2134.5-2130¿ét}JÀF‰Mçê_…À9xˆ3?ÈÀ<¸_W~l@†Cmqs?þÙ²"ý[
?°Ï¹Wf?²Gšs^F‡@¨Ÿr÷@)0Ôßù¿ïëC_Ñ ï?ïÂîþGn¿Þ¨èèŒF¿àcª2n¿á½?[_¢'¿à*MTAGNbll3FGL J2134.5-2131NVSS J213430-213032?ïòo›âŠ??RšHy
@€?&h'ÁGE'? ¹jó',?XS·âš¡?QžvÂ'³I?ï®o¸IGó?ƒ¡Šx¡N?4jNŠÌÄô?EªX.Sûo?ƒÀ¿yWœú?'ôú\џŠ?ïc:×?Ðï¦O¤Ó?ko¶e,?aäT)0E?š2TØy?€Ò%O?ï‹(×dÈ?q¾ç}‰Çò?]NuWŸÐ2?KÇ>'ˆØ?‰‹û"rÓß?p–_WT±‡4FGL J2135.3-5006¿ØcF'FÐ/ÀG3)¡¹ù‹À9-w9ó@ÕÀ<AÞÌ©'^@])DÇÛ @'bå¨eå?¨µ#§"Ç?²Ë›^ëÈ@"˹§V@_kó™d¿Ðð÷¹à`þ¿áîÅæ(¾e¿æÔ²¡¨\¿å§­ÞÊü¿çȈd½ïº¿íÃz=³¿¶AGNfsrq3FGL J2135.3-5008PMN J2135-5006?ïW¸z¿"A? çþN*y>?I‹™Ïw³|?MÎù3 ®?"<"Ù"º(? »ágc¸?ïŽÇ6Tù?'YþnB7a?G˜‰²€Ý?d©Û|&?ŠÔ¹iϙÔ?.÷v¸·©?ï7³o?}ÐúðŠ"Ó?g¡€$­Q?RZW@Í.?–*Yv³?|&`yn*È?ïÆ{Š
?d²tTGýþ?a"OA©â²?Q1Ão¥€?tOš$G?`Eærš4FGL J2136.2+0032?ÑV°Z7^ÀAÊdÂø7µÀ:÷Q۔çÀ<DFŸ@2΋hÔU@dZ˜Ó?ÀüÈŠrà?̙}jº@ FÇd®@ج8'¨f?æø¾&@Ü¿éòÚ/­m¿ç» !³ƒû¿ïÿùµc#¼¿î¬¢ŠÙã?ïù!bü$AGNfsrqOX 057?ïï¼?…øõ?eëOÒ¬ª?I&¼s«ö¨?XÓÆz?Sô"º84?Yˆ¶ˆ‰j·?ïl^Ù1Ø6?›rª7éS÷?T÷ÊB‹¹?iØaÅÜî?'$¨5œHþ?™j2%;#]?î5±S"9?"y7ñX?Š«3IÙ?€i̅Y¬¹?¦@¤v¯?
¿€"?ïáó7eìt?Z O¡U{?D†í·ÚX??úÿOE?hëGž¥"ü?WÏîw¢w4FGL J2136.2-0642¿í¬búK53ÀC¼ƒÛÂ3À:çž?ñˆÀ<l*YoÞ@bâ'']@6¹£$]?Ä%W'"(n¿ppëGÀF@ÃÀ0²$?ïÿ*þ~ð¿é$žoí#¿âŸŠÿøÉ*¿ìCžOá¿£¿Ïg¿Asè°¿ïÿüñýAGNbcuTXS 2133-069?ï±£LG?'ù
n¾€?Gù:fŽU‰?LôpûGq?'§sHÆ?€ßJª°>?î݉:o*–?¢¿hQ¡;P?dºWk»Ñ?€E¡é/·? ÛÆâQ¦\?Ÿd Մ:-?í9²z³zÈ?—	Mo"'7?"SŒ¬(@—?wbNåï}?³§ú"ß!¥?•:--6ô?îÊÃi¨W?†!Óxá?YŸç›Hþ?Qû§€'¢\?¢'Z( C?…™WáP.4FGL J2136.5+4259?Ë@æ碈xÀ:î}÷|¤À9Ê3°0´ÔÀ;´SFÎñj@RŖøƒ@Z—ÆZÂÄ?À† •÷£?š¦ÚtÖÌ?×vC=ÂXU@՞ñGU¿Öܱ±¾S¿äÁ/	ØÆÖ¿é`›š›ø¿á;4‰tˆh¿ïÿûB«÷¿ïX—;ˆBAGNbcuTXS 2134+428?ïäOªÂ*?}­Õh0e?Kþ¨…û?|»Ûú&?dÐVQ65P?c^C¨è‰Ä?íçËn†S?·Ë6À;šT?0úUÆ,.?V±Ñ:Ò.?°°¬¯qH?·±þ³X]?ír87"Ü?˜ÇyÍÂÓ?‡¤n"T=?y–ÙCâ'<?±zÒ°Ž?–hڐ¡ÐY?ïÖOÃrœ'?`!]¢q?0H–ÇBV?"Ò´»´';?sӔÚ@ØÎ?_bR¤zÇ&4FGL J2137.4-3209?ÅOQµ2ÀGób¯È°À;0vŒNW|À<®Úb·…=@ _Nã<û´?û0"|Ñâ¶?Òy˜\؞?Ìç±"_É?ýÚu+ü@—2[%@¿ïÿß´0Õ?ïüÉ_o¿ÖC™J~(¿ÖÜL|Z¿âi[
lпíýZ~{°ûAGNbcuNVSS J213726-320755?ïÅÂ
XîQ?o´§<¢Mú?HŠÏM´Þ?<vèaÆû?z
Ÿs!?nClà9ž?ï'nÛ
M?‡´>×?@א€ˆ@µ?R^ó´°Qo?ŠVÐ5rh´?†Œ»&™A?î'>¸Úĵ?‹<éŸ:Q?z.*'_¯|?jÜيsûc?ªFO-g¾¾?‰l­Dâ?îÝסãý?h½Ë»ËŠ?_}+'üðõ?Pj+¤8?¡&œ…?Ã?)/œ—4FGL J2138.3+3556¿ïå3	†€QÀ(w°ËæÀ;hájéƒÀ<}~´;@ ß³î¯u¤?ü±*ÇC ?ÎØLÈ/¯?Á>Þwšj?î3ÓÃt^@î¹[«Í?î½cm¢¿ë±K1Vº!?í˜{Ò7ñ¿ãÞ¢ýñ\ú¿×·†^ÔKÇ¿Óu3=šiAGNbcuMG3 J213809+3553?î}UaÁ‡?Ÿúø'E?Q‡l%¦4¸?I5njLaÂ?§¢H¶µÝ?Ÿ–.Է݃?ìœP°}z¾?ÁPuã%?`bŸ•h$6?s.½³!?ºšehèï?Á>¾'z4?í-FËï?˜w%¦Ù¨?w4=Þ?i¥Fñ†š—?µ$ØP¶Ì?—Yo.àj?ë·(CrWþ?¥åØë9
?g@xÕtø?g»›"Žwä?ÀÇUðSJ2?¥ã'nŒ`4FGL J2138.8-2055?Ó¿6™ªÀFì¿Â"OÀ;6ÍòfºÀ<ŸK·Žw'@!N¦.Ð"?øî"ã)/¤?ÐÍ>aº…?ÊÓ=ª/"ì?ü)T!ÀD(@ªL›,¿æ¯˜Ÿá²¿ä™Dàá6¿æ9¨bŠ8Ô?½)6@j£¿æâ
·'$¿©Úó+0ZfAGNbll2FGL J2139.1-20541RXS J213852.9-205354?ïdXòX"?‡GóI|-¬?W¿Nýæ´i?O åK`ý?'ñւP?††ByB"G?ï?ÙÎ/Ôw?'Ö¡ÚǗÂ?P™èë,?]tèk€º?—l›ƒrn?'òÓ¹*þ?íû{^®Ç?'œCVqÕ?vO7¿Û?krg"«{?­~hò28?,
º5¢6?í^KxAÝ,?™]>S7Wà?j&˜Jäq?eÓ¨)­o?´=	.¿y?˜ÛÂF»¨4FGL J2139.2-2214¿ïÎÁ»îûmÀG+'·þÀ:½-Œ*EÀ<f'}keª@ÎuÉ/ß@Ӛa?µø?ÀÉp·M3º¿²¢Øü0?ÙeèðïÂ@çØŽZ ?Èòdvw*¯¿ì=èîÁ¿à_$ù´Œ¿åœí ªD¿ïøÊ¿˜‡¿ïÿþ½à ¿AGNbcuPMN J2139-2213?﯋2Iž?'Ó½EW£Ö?dÈ`sx<á?_zMÁ†g?}Ö6¡·Ž?yŒ&óÞ¦?îÊ_hù­.?¡˜2'3Ï?`—Y"÷7þ?l²'*?¢P"×%¹'?¡øPÞFq?íR¹óŸˆ?—cñµj–*?"óëK"Í?ˆ."½½2|?°m5&WÎ?'€²×[`à?íÄ5xúØ?"È®fd_:?ƒ<Obñª'?v¥ì<ŒZ'?®ïϳçÉ?'‹@8Õ4FGL J2139.4-4235?ïƒ^+¯[MÀH*løQÀ7¤P«>¡À;=€Íù¦@ǘ°eŽ?þÞº))?•="½5øW?©(÷"¿P@@#L]¦¤D@Æu)LÕq?¹³V.4ñ¤¿Û:ð@ð¿àÈÎ:‹I¿Ýó§ªS¿än'?ßéà¿áyÑÕëYAGNbll3FGL J2139.4-4235MH 2136-428?ïß7ê9ó?bjÌC‰"¯?(Ýیr?!ˆÛa'%?o`ê\þí(?aü' –@?ï½
—šK/?¹;&ü?5¼ù›vãô?K€æÿ£†ö?€rL'}4?€º<u+z?ï!aAI´?«ÿLϚ?x~mh?{;"¾øG°?•´<™\ÅU?†Ò¤€¸–u?ïò5ܑQâ?LU‡TΤÅ?кïnØ+?Ó
ø?Z­ÁàÄï?L$Ê'"34FGL J2139.9+3910?ç5büŠ»ÁÀ$$ƒDÃ~À:^íLŸÀ;íGô‹W·@ܹ©.@¦ÜG©ã?ÍþAŽë–?¥äìź?׌4á߯@‡P&3¿ËŽ²µÊQÈ¿â÷Lg·Ÿ>¿ëõTáä·¿â?°"—©Õ¿ï÷d?ð…å?ïƒ/ÊÈæŽAGNbcu3FGL J2139.5+3919B2 2138+38?îrIÅî<?©÷¹1J–?eZp<Óϕ?g·]Ç;Þ?§‰_Óß4?©‡Ñ7"¢?ëà!—ck?ÂýÙßô?^/´)¹JØ?€Ú2Þ@ÎX?ÀC;jÿÂ?ÂÊíå
%?êH}稶?¨Q^?–¢+¼Èp?†CäÏk¦g?Â©Ä?¥ÁB|ÑV?ïqô¦MR?n«Íò?N`Sþlw?@}w¦†þ?Îh}É£?~à'nÞuÙ4FGL J2140.5-6731¿Ö€#¼ÈžÀDGë¿×À;&¸Lã¢À<ߺmN·ô@Z=~»œÏ@8ÇAr'?Ô2È?ïí8Go*Z@%žÀJ‹@uçâQï6?ïØB¡»&¿­}õ¤1x¿í…B>éÊ´¿ítÈ~ßY¿ïü•è41`¿ánß{ûùáAGNbcu1FGL J2140.8-6743PMN J2139-6732?îôkÜGKÝ?£`ÐÏ"?Œ9ó‡ ?"´±¸­Õ?"V¯ÀÛ?€èØfI_?âÙÈÕ´-ì?ÍFC´?ÎÍB(±?ʋ¾n¥Á?Ɛg#Ÿ?¹t~É['±?èWïN1kš?¬{f¡-´?»¤¬3œ#?£åÝÜètr?ÀÍì¾ ƒ‰?¥bÞÿ¥?ã3}; é?½úzznæl?ÕbÅ
ÐP?¾§™™…,;?°ÙÛ·?£')ï	§§4FGL J2141.4+2947?托Kª')À1/pyåŸ,À;»Üº€šÀ<u<;±'@u¦Vkq"@d˜Þˆ¶ó?Әíùþ?цÑ`/j§?úûs5X§@µ‡¼!ƒÞ?ëQóþ¿Úž+Cû'm¿Óä/à'S¿ç\cáPè¿á÷‹òç鉿ïÿïÕAGNbll87GB 213913.0+293303?ï:ƒ!R!?Œë)Ð}C?f£"‹-^L?^˜ÓQy±?•Û)dV0¡?ŠVl‡[@?ï'[•º?ŸFb°^ ?b½ÎK·»?qɛÑ\N-?5úÃåñ<?4ô@¼w?íuS‡Þ!?—$»ðô‡®?'<2øp½¾?ƒ¨§2K@?°Wó?'W!ŤÔ?í«ß·ïmç?'hº¯v'?qcSو,?c;УÅG¨?±ŠÍì?ó|©¡(4FGL J2141.7-6410¿Ô€˜_÷{;ÀE#KßÒcÀ8;"‹›˜À;ÂûB+»@Ðڌþ×@ÞbV6mz?œ5Qßµ?ºIؼKV@Z…‡"ݘ@ÇùZ"z?Üŝƒ‰¿Ýïâ+XÉ¿åwŠ~Ÿ¿äø¸BÒ¨¿éKʾՓE¿îˆŸ@¢‡AGNbcu3FGL J2141.6-6412PMN J2141-6411?ï0'4ÁX?"U‹#
+$?kÅ]Öà?'å‹´6?–Œxż?KЈ¨å?ïšÀ祖?‰ð¿{U–?C6oq"ì¸?b½ƒÃä?ˆhü]?‰(p1?îóZîË*?h'+ޗ`?ƒnSõàI?'56Þ}lã?˜k«ªŽ?Š2‰Î«?ïñÝeê¥(?M4…¦Ž˜?-vÙG9E?%ï´KÎ?X–YΏ?J÷5áLG4FGL J2141.8-3727?ï"öªõ?:ÀH‰GyBÀ9¢âž43À<F!*òó@9f­6Z@ÞÚ4"\?±Ë¾.ú>u?šwA] ø'?å	Ö¾IÚ@#ƒÊÐH¿Ö*¸¾«¢¿æá_¿æϋXŽ6¿édk"³Xˆ¿èt·,Q—¢¿ðAGNfsrq3FGL J2141.7-3734PKS 2138-377?ïø *Ø0?P$Y+ˆPL?üù~-?háAƒÐP?I¼õ¯}H?NAˆ0P¨?ïÁ€;%ì"?"Žè–e3?1¶÷ыêJ?P+NC¼?~$rïðöÈ?'ß/ˆ]çæ?ïJ*6¦[6?y¢ð˜ÿÛ5?f0ÿM‡™|?QïÎìý	?"ô™Aƒ¥û?wõ•ȍh?ïæ–А"‹?W1`6??F"Ͼ½0œ?:w±ã{¡Ç?cÇû¼(µ?T0h"³4FGL J2142.1+4501¿î_7I²ÀØ×à&EåÀ;	r£‹‹À<|CécÜ@ תU(¦g?úÒéF€?Ò¸D‹ÑZ?Ѿ ™'¯?û'fŸqJ@Þ«T4¿ïר¦Ó?ïû@Ô磿åʧ=Ç
쿼Gmý´¿ãCcaÏ'ñ¿ãтÿyGjAGNbcuB3 2140+447?ì<ÎR ?²ÎCˆß?bP€qÜ/?V~(ƶ
?½‡ygpþ?±ð&…ù9?ã?Èv̱æ?Él6ý‹¾?[Ӕ‰?s;¶"ã"i?Ùd›~_'¨?ÉF݉'?éº
&ÍÓ?¦jB•ülë?"ã~;õ»á?€*úø4?ƛ[Iü#?¤Kȹöì?ìÚ?ª¾7£?–æ6eôF9?{±½yF¢?mXŠþ™"?·ræÒyâw?–¯s(©¡4FGL J2142.4+3659¿Óáe…ÀÉ´À(Ïå†6À:x(E™gEÀ<Rñ¹_ä@ Äbr'æ?ÿ5Hyd?À]ÚPÃè?"/Àô½å?Ê@±ád"@»ti3uM¿éçkÅ?ïýTõ$Ú«¿êí¢ò(§¿ÌžnÀ}¿Ø`ÈðŸ:¿ä2jGâAGNbcu2MASS J21422658+3659481?îì« gj´?žå£¾ò5?YÁì=†P:?TÉû"I½X? g6—"C?žD®»^ƒÊ?ï…sÙøÉ!?šá‰¨ÉZ?1Ò
øـ¼?X[ôOn?Žy*ëo?š{­Ú¥?ìӊëCeƒ?š–¸ÀS?{ºaã´£?lA©¾K??·¨•f˜"?œ6à*,ý1?îÝJÜ£‡€?ƒnþmj€â?m¨JOaÇ?_a?0™j{? P͐ÕÑß?ƒÕU	r~4FGL J2142.5-2552¿±m'ŸS@ÀGý–áXuÀ:h˛teÀ<nÉìG¼W@ªü~ìC@Çùä]K?½Ùz|rí?À=
w}:@
;ƒcÍ@ãÃ"´?æ'ú㱿×Pâp£K¿çV±v/¿Ö}ê;ž¿ìÑý"ÕíÞ¿ï¥è\uKÜAGNbcu3FGL J2142.2-2546PMN J2142-2551?ïdqëÿø«?‰Ì:åÁ?b¼É#I =?[ÄÊs¡Tk?')[—¶¸?‡wÌ(MlZ?ï·íQl?"çÀúgA?3ÓÃ+ðÜ?L
'_úf?™¦'Ç•?"—û'&?î´›À8ü?¦ý÷£'?†ÔÀ_L€z?'³VÁ¾©?žÌXRŸ÷?…æoï¾Ol?﫝F?fñÇV(?^'Nyh'?M}Å䘳¿?SÖ;MW?c¸bÅÿž4FGL J2142.7-0437?é}y'èûWÀCä"&þrÀ:¿)h¯À<ẕ@tÀ‡o@ö‹AèÜ?ÈÛÁœÂîÓ?§®šÑÖL?ß¡/$°¹q@ÍåûŠ¿ã:;e0ÜA¿ã¤ñ@õh¢¿åõ²Ÿ$¿á%sW±N¿æ¨ Åó?¿ðAGNfsrqPKS 2140-048?ï¡Åír%?~‰!‡ž?R"o×Պ?J"àLЕ?…tܨ{é?|rþ§Óæ–?ï`ñó4s?'š=»-?B`²úªR˜?O (Hb¤?"N¼ª)?ŒÖ`3U#f?î=oz@lm?‹¸õfÈ\?x'23­Ç?f¹‰B$ù¿?©ÅU²Ã|?‰…qêû›€?îùAò¯©,?€RmÎÿY¿?e1,¬D?R®j­àÙD?ž6["uHÑ?€0âdÎn°4FGL J2142.8+1958¿¯‡3p²ÕÀ8c`9%»{À;°)(vÀ<ŠxËøQ@!q¹7C¹?ù_=?%°?х™ž!?ÈA÷[ÁœÃ?ù®} ½ê@	XfŽTl?渘B+ž"¿ì%ôïo¿ÄÝ·*Ï¿ÍØçø¢=­¿â?`A^D¿Ê4³{mÂAGNbcu3FGL J2142.7+1957NVSS J214247+195810?ïFD™?"¦–¿O"?E™D¨º¼~?Cß ]OýÀ?ŠáÚ$qmé?";å¥8?ï_¨—Þ;?'f‡äMÈ?PúÆŒu?vFÞ{›;?'ûQ«_ä?'èõT͚?î%H'¿Ôš?"½óàݘ?eTú P?V•ž€ÈM|?¬V-ãADM?"mòÊÔ]þ?íûÎdq¯Ù?‡æÂõ?Q'Pv÷?D"êX`?¯ºX~aQß?È;Û²ƒ4FGL J2143.0-5501?ã0û»LǯÀGh3Æ*À:·"òsOƒÀ<lꭈcç@jŠbo@…ËÀ]?Õ¦"»ë?ïÿšr¦ç@Ĉ'ðà¨@gIh~¿³Åüà!#¢¿æ¦²¡¨[Ô¿ïþdõM—?ïp¥ïé1‡¿ïÿìIiÖ]?ïŽéõÒAGNbcuCTS 0561	?í¨ÂÚˆ?À¤u-T³î?°'é7Z8 ?ÀŠÊâK+?v}M9"?'¹w©ÒÎú?ä´6a"¾)?Öj('?ÑêÞÐèn?ÕjSß÷'?¶F¡x–m?·ìµqî¢3?èçƵR©"?­}Jàx³?±ÙÆ%·?™jX_¨R?Ãt"¢~(?§»Ñr?êk{ÖǽÞ?ˊ†f™L?ĜµÏ™`ˆ?˸ÙÍàj'?‹U­Tz€?Í˜(]4FGL J2143.1-3929¿ïH}'róÀH¢ÛߏG0À9õƒ.I½À<W"4$Ê»@´çër@(¯œ:]Ê?´F¾?ì)4¿xÁ—©CJ?Ÿ±m@ôÙjM?ë.Áÿ"JO¿ÛWUý7£°¿åJàc'†X¿á'K3Úøß¿æ!ú[{PÙ¿ÌËc@A8¯AGNbll3FGL J2143.1-3928PMN J2143-3929?ïßòÌçŽz?b´/³GBÝ?3‰õ:´(?&jy"C@
?mœ9Ê/?aá¹Nvvá?ïɛÂAÀC?\^À?#©ìb"F?@ibÙ"Uæ?z"Ï|Õ`?~•g¾ûT?ï,ôš"ˆÃ?{Ðz°ª8g?flX
	ÎN?Q•o"gT?—"á¬-­¨?zÜ×…§?ïÂÄ\æ×É?d(ٞø?AÀ4â¹À?0kœ³«Z[?|eÊð<âÅ?cûš"I+Ü4FGL J2143.5+1743¿ï«"õ´¼OÀ:غ@ÙÀ7gþR€ÖTÀ;iÍ9VÍ@ù§>Ê@šz…\!?5…¦{2?£gQ×kâ@
…bÅÇõÍ@^'Š]'¿Ñ±U¢ô·"¿äâaÿÏY¿çRºýÂc¿åÉVAU¿è}ÿºà¼¿èÌ{n5gÁAGNfsrq3FGL J2143.5+1744OX 169?ïÛNþKm?‡4~´=°?:å'56D?2r[½™Ã?p¸–¨¶ö?‡, jäA8?ï†Xþ?—¥""û?V–'‰P¦?4¿æ?‹·æY¬ÖR?'‰`®~|[?VŠ¶±?•ñü$…?" %_-B?ö¦¬}ÕÙ?¢=!UüɎ?'è 8Ö"?ïÝìö&F?asy‰sñ?QBIÏUP@?NOÁüè]¢?iqäòFÃ?[°ÔÀ¶4FGL J2143.9+3337¿æ_–éfÀ-s¡ƒrçÀ:ÆXaÀå8À<iï¤h)µ@ aê»PR?ÿÑ*)Ÿ6?ÃZ°ûŠûF?«*n­+È?êpå^"
?ý¬ó@T¿ïù¥þÐ¥?ïÿû˜'2¿¤ÉlßÁ
¿ä²¥~Õ(¿áy‹X࿼ÚÝܔ•úAGNbcuMG3 J214351+3337?ï|Μþ€?¦§äÿExó?F<æ†Ê?@,¡DËñ?h—ׁ''?¦¥&¼r?ïÂáVè/?—7Úu³—?WšSñq×_?b£ãFÐÐ?šíþ–ÜÃ?–•¨½;d?í·™'"ìŒ?'þø.¹©?~H¨«ûØì?qžÞ_($?°^©aÞ?'Õ"Jb¥?ì†kaWÏ?˜ÚµMqk6?…É¡n¢?w©¨GEj?¹+A­?˜bŸžc)4FGL J2144.2+3132?ãjºŽå>;À0M>Õ'å!À9§<t$•À<+ºõ3ô#@S0 U @ƒ¼ûžqp?³êoJ×?­Y2Ý^%¶?ø"c¯ÒÁ@
<'A¹2ç?ïË}ÂM—ã¿ßAݨ[S¿àá–5df¿ãªŠLõ|¿Ùʊ<ÚPï¿ê) ¡`7AGNbll3FGL J2144.2+3132MG3 J214415+3132?ïËG™ƒ~?oInkž·G?CŸŸhä?5º¿çf´|?wèÏÑ$L?m¸j…[?ïºÎ*}A{?ƒmíëTí`?6AU¡´?FT@T1õ?€›ÓWôô"?' -à¹_?ïè"кU?ƒÇÊÅR?o
ÒܙõG?efŒm0£?œ3
Uv?°œ5—v?ï
W¾'å—?}³Îà­`?pÝ´'¬Ýþ?[°ÉvY?š›
ø€?{™‡ç¾4FGL J2144.3-7802?ê9†^m7ÀAuäõ8&À:l&ûíLÀ<£u»n@ôí}F}@C…%nN'?ÓÀ£~tÐ?ÐM`…ü¯?ödŽTÁù4@
3Ï.Pö=¿äþ÷Väd¿åv…}'âž¿ì"+
oÆ¿ïüë"£C?ïÂ}h‹…¿ïŝù¥žAGNfsrqPKS 2141-781?ïï¼_/¡?a¶t®ÇÖ?Cùqðuù?Fê\ü.õ?V‹
¹("{?\­ü)C9€?ïIuJìx?¤F?®?Z°ŽÙHQ?vE Ôú?•0¥Üz?¢IW]9ó£?ìlö¾Tñ2?¡¹
ÄT¸?t8"u.í?u+Ǥ<È?¸{;è;*±?ž° bø#?ïæ,'{/œ?j‹¤o6Â*>ó‡r»h*'>þ,zÛ¸»?i¬_ŸY"Ô?j'y²‡½4FGL J2144.8-1817¿ï¢Ð£WCÅÀG)ayWÀ;h¥IÑjÀ<ºqÊG·O@ ä²hG'?ÿaueݪ?Ì r}ËÞ?uH¥qzQç?¼ßŸb±P@vO[‡æ¿ïýQßñ—²?ïÿÔÌuŽø¿â
Ò¡"$¿æ¢f&¥†7¿µtSäوó¿â¿ý¡UûŠAGNbcuNVSS J214442-181801?ïØ(ÎÄÆ?kÚ°o^¶??4‡8€ýð?/!1Ûùæ?r£%qÊ¸?jÞÚvÂÛ<?ïƒvzªÞÁ?Š^=ÊÃ`¢?;$oß8xL?Oôé*†?ŽI=ÖNŒ?‰¸µ'V·ƒ?íê?Èbì?ÇɅ³Ð?u=¾]Ư?ht½ðX½?®´K®}5?¼É®â†h?îð¹Â
v?‰ßÝ£x?G4(š}Õ?D¡XYh¶7? —"5¥b°?‰åʙIòò4FGL J2145.0-3356?ÜÝNTºÀHÐGG"#À9HÆBoÀ<÷ïF4@֒­Â—@O,e¹˜=?©-ÝÞÂî}?¾&•Q¶@³w[0@»Õ]jo¿»v|3,RC¿Û–H¬A<
¿ãø#B$g¾¿æhH‰͟¿èÍÃØ1"Ý¿æ]THÏAGNfsrq3FGL J2144.9-3356PMN J2145-3357?ï|­&j>?'´
Çp³G?d×~ѨRÌ?aGW=Za?‹žÖ±Ÿ?3££^Rë?ï¿å3ߝ®?îºE3±?7&˜ïñۄ?Qßѕœe?~šü2
ú?Íؘ,¢H?îßìQdWR?p¡ÈA?8‡œÁ?~:]s5_Æ?›Y¦µP?Šð/u2Ǎ?ïîÎì;,?K!oÀ2?-iâ7D)c? 7:ßM?^¶«à¡!ý?Ivâa|ß4FGL J2145.5+1006¿ïïÚ²#åIÀ?ŒÌxéö©À;^.†%HÀ<§Î_ª@!í9Y=?ûY'ÿ?А›ëÙ?·Š¼+R?êϔÈy€õ@.-%Òø`¿ïÿÆߢèM?ïì~Bûþ¿Úd\åX¿ÚÇýsޟ¿Í–ÿöÅě¿ßôâ?¥²AGNbll3FGL J2145.5+100787GB 214302.1+095227?ïÖԑç­?rlþ½?*àOÎvç?6Æ29Ov?s¾¶1ò¶›?q5ÔKlƒk?ï|Æ»'›Ì?› A-]?4€1âȳ?K—<ºil¼?'ÆAc²?šß¸ùѶd?î¿	ùn?"
.÷=?a,–xÿÔ?RXKá|Ù?­2ü¤¸Ù ?"Î	ÍÀ ?îƑNFÖ?Šwäç^7,?DÍ4ñâ­??Ë6@hà?£C¹Ú«Ë(?Š'C/d4FGL J2145.7+0718?èGӍJÃÀ@´Â	$lÀ:µmÖPÚÀ<]¸"Üû@ q›#òÎ@Ñ|^?Åçþ×`ú¿•vFáÄ^G?ÒoÞ_FaŽ?òH›—ËŽ3?ææ¼Aå'·¿ç^-¢¥†ã¿é_ωþœ¿Ñéy«½ˆŒ¿Üœ\AŸ\§¿ãh4ë~AGNbll3FGL J2145.7+0717MS 2143.4+0704?î+£€™ìm?¥{Âk€
·?`¶âÀ´?cM¨—þ"Ì?¬:Yͅ7m?¥DÓ¤°f<?îA8yÛ
X?¥€'õ˙1?t‡OW#"?~<f•W'Ò?©[Žwjçô?£['ÌïúÌ?íYVŽ»wÍ?˜Yo%Ò?w첡nÍ¥?g¸®r¯9?³¶€`
T»?–ùö"Ï Ö?èG+fp -?ªÅŒw‹š?˜Ê,8'îo?‰ÕyºÝ?ËÊß/!}?«Bªö–4FGL J2146.4-1528?è·	'¼fÀFÑ|¯Ý©À:YyîÙgÀ<1£üÉêš@4I'n|à@Ì·ƒl?¿Î-_‰¨`?¿­0û›|?ø¥Èçdþ‡@ëɃl0«?ïó!3F¿ä½U¡E¿ëa¢ýpƒ¡¿é¡YìÛ`¿ëõ ޜØé¿ïÔ+{¯AGNfsrq3FGL J2146.7-1527PKS 2143-156?ïÔûEÔ¯÷?q‡©þ˜ò?Oß7'Ø?_?I¸!äDxV?q†v#lýM?p'ÅJÔñ?ïx­¡ƒß?'\¸É@³¼?HZ‡X7?YñXjj ?'w"Âd¯?o²s™m?ïš'WŸ?"'œÑ~ÿ?qá1}I\Ï?h皬?W?˜"aâµ?rÓzØá—?ï'w™õ¯?nr9þ%­é?l®r‹¾?W7R'ì	ù?"v¢Ó_Ñ-?ifÛX½j4FGL J2146.5-1344¿ï}†µU%»ÀFy—Ý÷wÀ8ë¼3øUÀ;‹Ûϟ$@Όïg+ˆ?÷ëŒ
dÝÐ?°y½!3+?Á±³ì{i@)4ÀÑìÇ@fûc
@…?ïGM1:Ç¿Ô[â¿Ó·'I%¿Ì¼&'j¿Ù"­‰'¿áœõ~DZ/AGNbll3FGL J2146.6-1344NVSS J214637-134359?ïSx'y‰?°û<‹?K¼é¾MÇ?¯'ˋÖ?‹{ý,¾'?‹ÍÈA;ýf?ññ5É?®x3½Ñ=?{²³<Tè€?žSóHIh?¢¯úybZ?¥§­ˆÛ?í(ó
_Êx?£êÆ¥e†?•
²uzóN?'}ÿjxû?±tû¢ïj?ž‹9ˆ­á?èAíîÿ(?³e;Ö#ö?{ôE™ÈR?m2–à©Ï?Φ3¸Ï?³Š'üúµÆ4FGL J2146.8+0425¿ÏM"%™öÀAµB€®IÀ:—Ù
LïÀ<3ycՒ@ò¤ø`@E"FK=ì?ÈèÁà_¦¯?Â4õ«?ò¸M¹Ç7@¶Å4ý㛿萘~'€p¿}è(a·Ä¿ê@õ~丿ëd&ñ'9¿Ç=Xlþ†¿ïÿÿÊPËAGNbcuMG1 J214653+0427?ï¹ ž?†#«ç˜%c?W݅¼ÍûÚ?`·Reºª}?}x–"ñl?ƒ~u~'Š?ï%)W?¡GáA@$u?WLj¬'³?stãñê¶?™ÞmtŒâ?ŸÇ6ä£/@?íݑÓ7ì?™Ë
PgŸÇ?âD»VÈ6?}aOkj?­®QŸfÏ;?–Æ<wH(?ïzPCët—?w_"iÞèÉ?I4Ìý#?A¦2Üj1"?Ø¢5Q¹Ô?v˪0´e4FGL J2147.1+0931¿ï1LÂëÀ@×ÆûÒtÀ8h5qÑÔtÀ;Ò!¯}0­@'š¤†ˆ@u…zþ£ß?¡÷Hõ™L?¹"ö%j@t¥ß"9ç@h[J©q~¿Ï"ϝŒ˜T¿ãSßà›¿ç·|¯Ý©¿èØÍ÷o7Æ¿éd=ÔÌË¿èÈgÕÒ/AGNFSRQ3FGL J2147.2+0929PKS 2144+092?ïÒö½¹x?sr›5	~?VQÑ⾏Õ?d|ýô¬¼4?pð,ÿs ?møºèpG?ﳤ¹¥Òj?ȚϞ¸?A•lZX—?i_Ú1i	?ýø?Å¿®?‹Õc<j?ï"¤,[Æ?†±6ÃNså?x+7ÿiZ?v·|H@Ùç?•¸€¬t¬é?'óñ
ÎP?ïó
»ÒÂ?G䯕 Ù=?-&¥ "X?$BJäö]?V?µFX&?EÅ
P,_84FGL J2147.3-7536¿²,õ®!ÎÍÀBDR½<6À7™I¬|À;Œ›aöK@ÅeÑÄ®@íüºÑ!Æ?"~<*©?±>uf3'@;8 ؽœ@²\L=Ý¿¹¦'ác^¿ã‡>ùºì¿æ18‡0
Š¿æM= t¿ê‹P*º¿¿éWòeÊAGNFSRQ3FGL J2147.3-7536PKS 2142-75?%®š?ƒvgbiñ?XŠZk;?PîÛjQ;z?‹ÇréF?'³löÆ?ï©Ë]µ¥K?Šy¦*=bÌ?C Mir¿?]
_¶sË?"[ Àµ?‰VtKöb?ï<¬ÏoP?†ºíL4Ài?}ûè}Ý?zZ…¦¿<?ëkòÛäâ?FáBX?ïûQO5?5ïzFuëƒ?N`y?Éó?…a!ï'Þ?@0.´—18?46e¶Òáñ4FGL J2148.0-0733¿ËãÛq5ÀE6€àe0À:S¡"I¦<À<j|>>ÿð@¤—»H?ý_ÂÞ6œ?Ä	Æ'l*¡?»JµA&!8?õ¶{ò¿¥@5˜þ")?ítM_.cÁ¿é§ ÉN=¿Ó +ïrC¿ÖH´å$‡t¿äú¬¤8Y
¿äÌqæÍAGNbllSDSS J214807.08-073347.0?îÈF±÷¼w?":¼?"¯¥?Y&gܼ?Kp·'©Æƒ?¢²»­EW®?"ìNtóZÌ?ïGÆ҄ë?'ËÆkÀã'?SëS×)Ù?]…n%Åï?œ8Qè<Ðù?'3^­=Š?ía엊
•?–ËmKzd+?{Èò¯¸]B?j¥6êW}?³4´%…?•Pi¹ÃhÌ?ís;õÜ°P?ŒÝäsî\?z=S•§?còu?²½eD)?‹‰Yqºñó4FGL J2148.6+0652?äûc¯ì†ÀA™í|o½À9ñxKk8]À;ô÷Zï:@Q·&tU@BªA‡‰Í?²•>9x?ÎÃ핚0˜@jgÀ¹ï@
`ç\ðñÅ¿Ê-ªÞ•I¿åÖ]9–úƒ¿èºk5Øÿá¿ëƒï¾"OÙ¿ïÿúŒ—Ó?ÛÂð?˜œDAGNfsrq2FGL J2148.2+0659PKS 2145+06?ïÝé³ÚÒ?ks\¦‡•?`™'A|Ï?_Wñt¹ÎÁ?a|Éã±,§?aÔ‡x:õ?îŸþp\žÒ?©´3y|ÞW?tºB駾?Šbù"uÃU?£hØqØÝÜ?¥ù4jk?í­z¨?™¬6.³¬?"Šî©2ìñ?…G[7%Ð'?ªâçë\u?"a\®£‡?ïf´ï›Ž?'TPòGT?s^"p°+?`l'•'ôv?š;¢½0b7?€ìÑ)5Ãy4FGL J2148.9-0121?áVÙƘÀC£2œ4~À;Ïëe>HÀ<YLÓi©@Z$×$êp@ºñ-À?Àî^—ååM¿µ"ÄÐÿâN?öÃBZ£‹?úäd¬R?îŽñ"%¿äCHT,§ÿ¿ìlü›Ç¿Ü¨¡õ2Ç¿Ö5²~íÆ¿°Bœ ¡O	AGNbcuPKS 2146-01?ìüÁa»ý=?°Ü©|kyÝ?r£è"˱¸?h°é¯w?¶ï¶oóZþ?°‡ÑÏVq?î": ™?£¼Ý>ÖÎh?j¤*-}‹?z,]»¥$?¥$ECŠ?¡ŸÙ—'°_?ìðf5D™X?›‰°1f2?zY¹×ïõ?hCËÊ=?¶×2ÅM¶3?šRËGÆ5ï?ë£]l3T?¥1-¤>C?{0Ãdó?s×æ>ñI‹?À™4;?¤œ"K\4FGL J2149.1+6104¿ßÑ׫–!@mœBÁE°À9®cÂG7ÍÀ;{Š '§@©ù
G'@W¬Óª7?ávŽöS?Û	tBÈ@ò³Ù¶À@	ٗ
ô¿ÔÍÂ6Ƽ¿æÛz_A®÷¿ëáûbó¿ê(úãe¿ïb>ï)'¿ïŠ‹>‰AGNbcu4C +60.32?êb	6lÐ?¾qç{m?£fóoO­?££¨Uâµ?Á ºÿR‰?»DA¿E²?ØZX²²à.?Ðk¸©Mí?ÎÇ0i–…?Êÿ¢—Q‹"?ؘõT?Ëßy̐"Ô?â£^?²ÇíZÒ*?¸ÿÐ²
¹?¢`?¬^?պى•t•?±¶†çÄT?á&cµðN€?¼wåìã9ÿ?µš£ýóÍ?±YÅã26?ØLµkæ?¿•æd²›14FGL J2149.6+0323¿äÙ:;¡RÀBNpCßÀ9Üëô°@¥À<F։äð°@ú‰*`¦´@êOyº×?¸N\Yr7*?«yQ'æ?ñS(ýOL@$xy8{¿¸tGz'î/¿çOš¿à±Šâ¾w¿áX¾]g¿èöTOãm"¿Ó[Þb¡_âAGNbll3FGL J2149.7+0323PKS B2147+031?ᅯ!ÜÐ?qÅIÌ°R?O­½ÚJO»?DDaD)?|?ù³ÈMâ?pb¹$-Ák?ï°pëìgr?'­ÐäÕ?)ùv	Œ»H?:†í0i?ƒ{ß,¿ðž?½2unzá?ï4°I#Šc?}–¦))Ù#?imkµÔ–ß?cÆ}©†öe?–<IdÔ â?yI",*?ï‡À躋g?r?"3ëvR?Sï•ÌÁÃr?AcLW·çe?‹'ÓÄíú?q†lNýUd4FGL J2149.7+1917?ã͕óØærÀ:ZS2­À9ë—i=±;À<ó"Çz@4K¯«Ô°@·Zï9ß?½À©}è88?·Ù\Á殏?õ°
fóT@%÷5¿ç•žˈ¿ÜX'¿Ä¿çOÁ´?ã¿éxM·‡¿ãĀ˜@Ô¿ïþž
ÇAGNbcu3FGL J2149.6+1915TXS 2147+191?ïíZQhϧ?]"{…]™?0}$J$t?+ÊTDÅ¿?`–
§û?[ËqV½þ?ïÖ~ÌN?xú´9+\€?!¢óȚôæ?5Ü×Ë°?tk)ZU ?xXóh»×õ?ïÁê½s¹?†) Sü?püš@Û_6?aÚ+àœÁ?›(œ±?";ƒ¸4?ïÇ戍|õ?bh	'ð?>Ç°Ê>ã ?/"ĉ¯h?z @¬—?b!aw"¯H4FGL J2150.1-1410¿ïWôÕ÷»ÀFö5"_õÀ:¦‡¾¥ÃÀ<1£Œa¢²@ ×ÅiV?ù»À6âë?Áb@|që€?Â2‹˜z	Ü@€	ö#l@ՑíRÔ?îyˆLj;Þ¿çká©Ó¤¿µWXvb¿»^¾Š¥ò¿ãïî:ތ¿Ôéâéj'AGNbll3FGL J2150.2-1411TXS 2147-144?ïãVŸx?,ë.·Œâ?f
ñZ'?`rLÀ|ê?œ¡×ÍGh?Žgà?îÔyuvđ?›þ£y ?cÎåœ	Ÿ?p€SBBœ?¡{zNÓö?š²¶©o?ìÁ(V:w?ž½ûä›^¹?ƒME¼??s –~˜?·&»´?œyüwPgâ?ê
!ÞTŠ?£4É-Yp?'›¯ˆ
&;?o"¾Ïf#Ø?Æ­½fq?£®³Ãõ4FGL J2150.7-1750¿ÖaŽaz½ÀG¼Û¾WïÀ:R}ü…!=À<ZS¸ä¸|@<pšœÎØ@2M	žs?¿Ã±ðþZc?ŸªžÆ÷m,?àv©ò´h@·FRʨ?ïî6>€nO¿ç8å#Û§[¿ç§¿Í
	n¿åà½D™¿äÍcˁs2¿ïÿÛb;ßTAGNbll3FGL J2150.5-1754MRSS 600-040574?ï.zÄÜÌJ?š\o¹OÛO?fVI_Ùã?eé¯Vxì?—eÞ8kSÓ?˜‡	~Š¼?ï<A>V-?•ájûè?Puk\½z?\PÁë%ß#?—e"s^~?"@8¿…?í}•áô+‡?—Å·S>?"YñöAŽ?sdÐíò?±¥²ۚ?"ðWZÉœ?ïjQ¢ƒu?|›kA•ƒ»?rf‹eÏÑÛ?`è­gä
Ñ?˜™ò;œø?yN@y+4FGL J2150.7-2810¿Å±ƒ Â~{ÀIâ`²È?À;^Ý÷—À<",·/¢@ 6üªàéº@%…EN¾ª?Ñrª?ÄÏi_?*¸?ôKà©"£™@ì&ØÜÐ{¿ïþÁ?|?ïþtå…*w¿ãàH	"
@¿Þ¯°ýcmŽ¿áøžö{¿àÖv~â^/AGNfsrqPMN J2150-2812?ïÚfS/aø?m³™juÿ¥?=ß8O?<g""T¶?pîâænÏd?kµ¾Vd&?ïŽíà»rU?‰)öéüÞ?=͙{fX?ZoÓ°àÑ?‹V·|?ˆ–<–¼«?î±uÌ'?Œ£7Yè±J?j1&•²^?cc@>Ó`5?£EÔ4‰ö?‹;·	
†?ï¦+ƒ\™?….î>—M?W1X£F?LaµxXà?œ¹çz
8?…('ݕ,4FGL J2150.8+1118?àõS2úJ¬À?»5*"8	À:å!ÁçãÀ<2\sž]@¸ˆd@H{Ã?ÎÁ".öŽ?¦cžœ?Õ=îãx	ý@ý]žk»e?íÜêâ6–j¿êåídòÈà¿ÙziÓe¿ßÀâ³¾Þοä´Ó˜A¿Ñ–éÜ'2ÊAGNbllNVSS J215051+111915?ï	«å*"h?'y¸$úŸ?JóÕ}jp?=D8ˆÉ&?òä®Ð_Q?'KÌ^É?ïEè&?"»ä):òÞ?Kƒ cÉqš?]¨lK–A?–ƒ£_Üâ?"û1¼z?îçi]å?]cmSþ‡?qGPµp?\·ÃÒ7vï?­¸­_Ss'?Ÿueƒ?Jqà?Å­íÍ´??[øu½¡¸?Iÿ®,çhS?¦Në•84Ú?Ì1­Ì<è4FGL J2151.4+4156¿í•ÏrkéÀ"͒·þ¯À:_úŒ"¸'À<Ib(D€@ [ÿûù5?ù´ýö°Ì?ƙähŸÒ?ÕNŠø.%@«dÅ|vs@ø~©©1<¿é@¸Azsº¿æx6ÝâžÆ¿¸ÆÚVM?¿ÐäK3''¿áñBwô®¿è>ôÈAGNbll3FGL J2151.6+4154NVSS J215122+415632?ܓ›ÕMÔ?Æ #2ì_í?¤ž—<‡?™¶^³jW?àlPü?ÅĜ&بS?ätKm ð»?Êll£(j?ö'Ðã?"ˆ_.ˆ'?֏`=
?ÉÿÁ˜íô´?ånC¤`?°(¬îèW?½ýXŽ‡à?¥V—
lK?Ë~rË;ö?§Ãӗ‡æ&?é^úž±?£³¦ÝÃO?…WKS9=?t™í#gšT?É0*ä¡©?£q<+½¶J4FGL J2151.7-2749¿æ»à'óÀI-ž×ÆûÒÀ:ªDkiÛfÀ<0®û*®)@Ó/Â"'@[*'ñ¶'?ÖómàÙ??á4±¸tP@$è'4ù@
f´¯Êˆz¿àÃNžÉ"C¿å–Û¿
¡¿è¬R¾éµ;¿ê¢"FY¿ïÿþøþ"?ïòª¬çT8AGNfsrq3FGL J2151.6-2744PMN J2151-2742?ï©cCƒÇƒ?ƒ1^ Ÿfú?Qu´‡?VkL)>ù?ƒuŽÿhŒ?'4þiÒ!?îtBWí¤?¬d®å1Ó?{kJP_E]?'.ÏþFœ"?¥Pòu="?§u]J>^?ìÒëﺮÕ?œ9ﯯ?™äÞ×ö<?†6—AŸ)#?²ïhÌ,úP?—€æDç%i?îbA°¿>?–N¦³Ef2?Tß.Ä7ò?Jq†804ÿ?©4ë}æL€?– ÀUÑ4FGL J2151.8-3027¿Èý(":ÀIb@îÙÀ89ÔñhŽÀ;¿?úÁҞ@æ°d@ýÙ<FØ,?¢T=nöWá?Ç°|ʀí%@è_^4h½@{Ã;~†C¿Ó¡ZX;*x¿æ‹a]¿ë¡}¾œ³¿ìàYq‹^¿íS›R×=i¿ïéjÇôö¸AGNfsrq3FGL J2151.8-3025PKS 2149-306?îâ²Ø1²"?¢/z£iÙ$?›çCÓÃ>Ñ? ,qO™Há?	"˜óý?€zÞxt?ïrû4|®?•¨
uÁ?]ìÍP
þP?€(V•
Žâ?ƒ™Nßu?'¾ÌSš+²?ìRFRÝêÅ?©t$²NíÅ?®PvÊC9Ù? Í'0Ù ?¬‹$ÞÒ? 9 ­ÃÕ?ïáŒ_ßį?a‰ÚdØ´¥?T]'¼Ö…?P.¹šð?dDÖÁÐF'?ZÅOô›4FGL J2152.0-1205?퐰84ÀF¹‰›õ"lÀ:Îÿ€¾À<k¹›— ›@ #Ýqµ¤è?þ%鞔«?Ñÿm]ü_?Ë!]•Ç?ýíG+7¼/?ÿ"IŽ¿ïýPÒ8r?ïÕ}«&‰Ø¿àÛá¨&$W¿Ûf®_ÏH}¿áP«>¡%¿ïÿä¡Õ¨>AGNbllRBS 1791?ïŇÂʗ¢?p§NæS‡/?Jċ¥v~	?Azñ¨ùM!?yã&_]?os8œ¨¾ë?îðQS'Ô?™êé5aƒ?aªæÚS(ë?k—€ÖÆëÅ?ŸÀxÃÃ@T?—ÿqRp'9?í׫ý	®u?"Ǭ÷™¦?€ÆÇ¡/~?qƒ±MKÙö?®SŽG9-?'ZÌÏ¢Å?ìœéÀ5A?˜JÿKNmU?ˆ8Wž½?y&Xñ%–?¸¬@}B!?˜'"´ÆP4FGL J2152.5+1737¿ÀçHŠ®À;°¸{Üð0À;óiï‡ãÀ<aŒ¤¾Ê@zo÷ß @å^¼Mùˆ?͇4|´['?¢tâCñ5Q?ҝO0¿»l@ŠšrÝm.?é'Nž·Ì¿âZi7Ñþe¿æ]¾Anµ?¿ä$à¿ÈØL¿ãÎAvÂÔü¿îô›GðAGNbll3FGL J2152.4+1735S3 2150+17?íÌb}º3)?£Êúi?aZÃÇiI?S­f¡Uì"?±ùÈ+q?£bdð,?ïeف×?"´¨ zÀÑ?Q΄«¤\?]hk‹UD?›–\….šý?'Ú~'y—ï?í œP¹?"éýÝr?{¼]žòá?fK5vÏ»?±Û9g HÄ?"™]ØP¾?í N
/žK?ƒÏaÍl?f…ºÄÝ?T"O½Â?²Ia˜¬æÁ?µ®\ÓåÀ4FGL J2153.1-0041?ìA5ÒÂ'ÀC߸ä¸{ÝÀ:é€æDmÀ<oèPïÝ@!æfRDpr?üÿüB?Äݦ¨ É?xCGŸÉ*ù?¶»]û)@txÍÇ?ïêLÚ¤%å¿ë^°ô)2¿œ›œNª³¿×«X¾ˆ…¿ÛoŽ˜´—L¿²WxÅ8¯AGNbll3FGL J2152.9-0045RBS 1792?ïh!ò§B?ŽˆÄèÒI?2ÌeŠwj?,³ávu¿?'°«Khíï?ŽO•ÝâÆ#?ïu}Jâ'd?Žá‡†è7?B~2xn"6?Tº³@ÙK?¼eêbR?'=J9Ñ(?íYÚã¶ò?œ*<Mt?g¹Ai&0ö?Zš‹hL?´s^ÛéÝ?›ßöÊ÷Ž?î×#h½E?'jl²}ª¼?Ræݪo³É?GÃÒ*	ùW?®VÜ ®?'n·²$34FGL J2153.8-1137?ì…?RåÀFÏËÉdcÀ9JÃÿž±1À<çq"Á@Øi¼\<A@7bR¯'?­'n®ßQ	?° ½ ñ
?ü'*߈'@›†é_¿Éó£»±q}¿åcn.±Ä3¿çBE¿é}þ."¿æà+²~m¿çÓ`žü/AGNfsrq3FGL J2154.0-1137PMN J2153-1136?ï͙ÄÏ@¿?¿•ÏÝS?8hd¹7v?F
ŽÏ?w¬—W"
_?èx¯`ö?ﰝ‰Z‡º?‡¾~¬Ç!?9¤1S6t2?Sx½Z9?ƒ|Ä^?…v™û#ŽW?ï8ðÏëÍ;?}Ž~KW?gº!ÍÈ@Ý?T(Ñû}Ž?•ê¡ÈÍP{?{r""–Ca?ïÁ‰sÊNŽ?eö¯ÃN?\/\¤ù²+?MŸúyÔ¾Æ?x/nñšLÒ?bⅇ̪N4FGL J2155.3+6602?ì>\Ò=úâ@"	¶o"5ÒÀ:êg¹MÀ;²ÎºÖ¨@Iß,ö®@p'ݽ¶?ÉÅ?º«3?ÈóÜ܉0@γ!*3@Ý:ÆF¡?Ë*é£OA¿ã7ÊaŽž¿êdkð"ò¿å¬"½ð¿î÷à†=¿ïÚÀ«VZ€AGNbcuNVSS J215520+660839?ÞIè(Å?Ý?Ä»h‹¶Š?²àWɳŸ?¬MϦJÓ0?ÜþäùÓ:?Ådó^¸^G?ã¤ÚÕ?ʦô/'Ås?¨zûH·?©ùã÷YR?Õ¨€Va??ÉL
G/wŠ?äŠäëåt?°Xnµ©?±œõL¼¤š?™D	2Y%?҄¶âùó?«K©,k?åØŒD@?¥Í7C(ø?²ÿ´Ž?•"غ¿?Ðbö×;?¤Êzàn\ª4FGL J2156.0+1818?ìR%|'KÀ;Èf^ê–À9æ7UãUÀ<-5Ã0l@!ŽsöœÕ?úP¿54•3?º‹ÉwWÐL?¸š¾²­¼¼@:g9Êüé@ù0´¨¾¦¿ê?ßÿY'í¿ÂI#ŸíE¾¿×yTŸêk™¿ÑBõ"ûƒ¿Þnê.£ˆ¿ÒÕ½aIñçAGNbll3FGL J2156.0+1818RX J2156.0+1818?ï…åek}˜?ƒGç[˜(´?TY¸¼…ÃÎ?OI툠4?‹ûoáƒ?'%ýSÄS(?ïQµ·©Ì?'ف)s=?U¥ÿš)Í?dÂfóÿb?"n÷ZÒ£ã?'w{ÍÍk?í?ZØßÂ?™¢¯Z•b†?'~'%Îz´?r¹Y‡‰?³µVôH ?—Ç
ӓ‹??ì¶Ù£_*?"Äô¾‹U•?{‡]ÆÔkˆ?iåÈë€ò?¸–ÃVw¿ñ?"
÷÷…LO4FGL J2156.0-6942?ãN¸Z'‹ÀDH—žÖÜÀ:T}á­.¢À<((@éÈ@rK'ÎÉý@Eþw?ƺøcÿXæ?Ôûñ}†=œ@3öÂiœ|?úpH»ÊF?À *Aò闿ÌĈZ¬ôÀ¿êôZ5Ö|¿ïýA©î{s?®-ýê&$¿ïûpÿqºAGNrdgPKS 2153-69?íûyN~û?ªF‰L?•æ3
YI&?˜h6vA?¥UM"kk¶?£¨‰½{™?êóތþÖ?ÁŠWì¯<W?¤Ø=Ñj:r?±§ñ­»|
?½ûb"âì?¹mÓãDž3?åÿ'šëoí?«iγãKÄ?»¢Ã¯Sþn?¡äâŠ?Ê0S¼¨A?¤‰û	#ûæ?ë‡Øä"\b?ªˆþ)9—Ý?žùœg;.?™DóçŸ?¼Ô÷ÓN?¦W²ù\Ó4FGL J2156.3-0036?ךQ›ºAkÀD+¿@OÂÀ9é Ï¨À<3ëGWL@+ót¡@ÜewS?µæD1?œöCW‡j?åB]"<@µýM?+¿è è½ïk¿Ø.}`ä¿æ'S‹'¿á' ¹Ée¿á~ˆÑË9O¿ê–ÿ5¿AGNfsrqPKS B2153-008?ïâ•D²BÇ?b\ [–o%?3@""t}?&֏Þ)3ª?kª»Nª[?a¢é(sŒé?ïÍ)(ÒF?DBóÞÿ ?#Íí¦N??F}•Wu?xã¬ü)ª?~ÓÖp²?ï%ªÌ½ô?€¸ Akæ+?k­
i°6?bö&[4"?—Ö©[ƒ?}ʓ^ó«Æ?ïÞF*aÀb?V™DFE£?.&\/)²? öµ]h¯?o×oÛMK?UæW¦Mz'4FGL J2156.9-0854¿Ôµzö–JÀF]xÀ:"¶ÂŸLaÀ<z™_·ö@œ¾¨Fۇ?üâqy¿ß?ÌÙäwä=,?ÌMbI†@ê̒@p"³¬¿ÜM[=…¿åÅý_çœ1¿Þd}§ö¿Ù)*›´üÌ¿àRh' Xпïù–m•/AGNbll3FGL J2156.9-0855NVSS J215650-085535?î².#"ô?˜lŽ;i_?jr~ubÜ¢?`w#—ñ?£5õఒú?—Wé/9¦?ß**8?¡ƒñlSä#?d­Y´¢m•?jíe¿µ?¥ËÌr5©? ø16¦?ízJÔބA?—fƧo•V?‡$Í)?y»Ã@Þ?±I³é›?"ÿƞȆ°?ìï:'`?"z$ª~Å?v[4ŽWN%?efÀ»v?·"J↠?"¬¶¹z4FGL J2157.5+3127¿ïñò"œÀ2="ôÆæÚÀ8I"ðÅÐYÀ;¬šÚâ9F@_t;@_‹Íþü?¡aÿÏX˜?Á|®¼Áfè@ c7ë(Øf@xhZ†­¿«Íÿý¦´_¿à‰¶b'<…¿ã'7oØÕð¿åU¥ïqó¿ìž–XœyH¿êÒxþn…oAGNfsrq3FGL J2157.5+3126B2 2155+31?ïà«q…?"°ªðH?ƒ6nW=?">VMJkÕ?"ȳróIT?‹×ÔT&}?ﳊÕö›ù?Œ‡é‡‹*?C
©I˜?\"1Ò»?åY§ÇÝ+?Œ#4+è?슼¤?¦œxQðà'?°klùeí
? «@ãH%S?¦}eËÉåE?›/_EÏ?ïÔ%ØóÀÿ?eíi¬çÊÅ?CÐŬ?8_‡*†ßØ?sŒù…æݾ?dËÛ8Ъw4FGL J2158.1-1501¿ïRT7Ý|ÀH<ÈóÀ9G+ý´Ì%À<"?ø="ß@'€ vÃ@¼w¯d?­@
‡‹ã?±"\éü@]Á@ŸS²¯•.¿ã™*GÒ'¿Ú²Í\¿ž'¿ãž¯çÜô¿äRÀí ¿âi%'×µ^¿å-c ŽUnAGNfsrq3FGL J2158.0-1501PKS 2155-152?ï"aû××?¡Úóm­?>¤'"vÀØ?P®…Æ—?‰ò\u慘?¡XæV§{1?ïwñ¸à¢?'
¦¿gy?Gº^ö%ÔZ?\ƒ¡…ϧ?_Ñ2½=? º˜4jo?猪Ù?…°w8s¡ˆ?pq!ÓYü¾?e­Š×'Ê?›Î¤»Iež?ƒï"Uäâ?ïFakÿ¤Ê?~
¦Ê×?hiæÛ·?V/=Ç?"0ÅC/ïø?{{@c.Bž4FGL J2158.8-3013?Ûõ26ˆþÀJ&k¤"ÉÀ6A7Cc,À:p¢¨6@Y'¹'m?üDÄö>¶?‡Ñ)ëЍ?¤ùÖp9£æ@tBÇû­@ñé…Àè¿¿âÈ6ºý¿Ö—¿¤Æ¿Ü´žØ»g¿ÙÝF'vú¿à;`ÿX±¿ÛՀºûiAGNbll3FGL J2158.8-3013PKS 2155-304?í+gÆýÏ?´2tCì?>vÁJ¾?>b")†ls?·€.}SŠ?´,(ò‹R™?ï¤GÈðÑ?Ú¹ÚžÖj?Gpú .$±?c^Ícv;?…vþÈÙ_?: ÍaÖH?êçßf¿Vç?¬<"â?ŽÆÍ"™e?‹»`–±ðÞ?Ât'Ù?ª¡8kàs?ï½åìmzJ?u.W23û?%#tÕœ?!tŽ²r?€1÷*ñ?uë£Ô4FGL J2159.1-2840?Ç͍MA8ÀJ<³åuÀ:ŽF@RÀ<AôÚ2@ C¼¹Ú+Û?û<\ŒÈп?ÁDœg)Z?ÄX¾Š@BíJ.!@vðéa­ð¿ïÿülò?ïÿÓ?,» ¿ßep½Wcê¿Ôo……t¿ã#-A+ÄT¿äK"=,®AGNbll3FGL J2159.2-2841LEDA 3218689?ïÏRÅÍ´?yYÔ®]ŒC?V"	pÒC?Q%½µùc	?rÕZ¼ðñ?x‹Ê?ïw[´üMI?'¥?XÍÚ¥?M	Y½Cíº?a.Ž"Ï?,>'Œ7N?Då/¤ék?î<JÁ¼Õ?'}YÒ?yÈu«A¶?kė^U?©E4Iªt?Þ6ƒau'?î&GGï?‰@Â	%Å?|R-ô³çB?f¨m}4Hå?ªÅÌ÷¤5?ˆ¶(.-4FGL J2159.8-4751¿êö÷€—:ÀImÙ]ÔÇmÀ:zê÷Z?À<ƒdIU´g@t"aS×î@(?NÊhn?¼í™I'›?" ë!<¢?ÅËÀæå@¿Q$_Û³?ãÁ­Ÿ`¿ãà%¿­)™¿æ9Áø]tO¿é+f ïÀ¿ïýŠoZ*ï?ïßM œÃAGNbcuPMN J2200-4751?ïéi…¡Ãb?bp./'Í?6¼5hT?1Ò[<–?c¾ó®O›'?a	©1ñ!?ïµ:€"9†?†z÷2·?4aå–Ó¤:?N2j?'P®{e?…~õw
à?ïCV›ïíÞ?yò7Å{ØÚ?h0ªR¦]k?UXmÿ¤?"7­x‡?xlñÑV¤?ïêZ¢¼fë?Rθˆ£Þ ?*ÅÙy"?"<1ÈÆ?cøÿ¬R"?Qòw‹Ê¤¶4FGL J2200.1+2138¿î±BU˜–mÀ:>$þ½
À:-m÷T`À<KvY"±@.WÁ²èJ?ÿ¡mµ?¼×Õ˜8F?°R,—Õõ?ô'p*4†ð@)ˆh™Çg?¾†ýOüm¿Ý-£ùnì¿åœº¶IӉ¿Óú D¯¿áƒsR3Ñ¿ëwÁ½¥AGNbll3FGL J2200.2+2139TXS 2157+213?ïå_óM?]ÂJ1‰\å?1øðZ_?"k`º˜­q?h|*"Vþ?\'ë'0µ?ïƙ/~;c?€ÝäÿŒy?(9—ôF<*?A§¯à™Ÿ?{ñ›@Ï?Z£Œ˜?ï.
ƒ´«Ç?~Ø¡qLô?f+m»g?`|–oÚß?—xíGϵ?{'Èy&*?ïuVzÔ?q•Ãeµ?P']D\?9°ÛÃEŽ?[+¿\_³?p¨Øt4FGL J2200.3+1029?ï—Çñ,
áÀA.@…+NÀ:x3|.NÈÀ<PX(¶¯@¶Z
'º@ISù|X@?Áñ"ÂÅ7?ž¾}‡Gåû?Ú¨Ë%WÓQ@I$ß]s#?ïÿûB«÷¿äÜ)áû³¿ê²îO'¿×ôè_Op׿éL÷?7á¿ïÿ¬)ÜrAGNbll3FGL J2159.8+1025TXS 2157+102?ïƒËAÿþh?Š$¢š†?cT‡0ó"n?^{¥''V?Š8
³Ã€Ú?ˆ®#X'š'?ïóOg¥€?œ±ˆäß?\y‰RO}3?jȳcÚwL?ùý}æX:?šý5s Û?ík;:×®?—
qõ^?…Ñ&S_Û?xjÒNM²‹?±ì^Ün?•E'q7‰?î¡~£®?ˆ
C¿-??‡"*ýš™2?x
ö!Ÿùl? ¹>Ù?ƒ‡¾«E 
4FGL J2200.7-2414¿äÅP4SwTÀIÎWâ?$ÙÀ:•'Àa"À<'F…@J'KÇ~¯@e9Z"¡?Áþ{
ã3?©¤2|]?æá¤_Æ95@
Ô‡Spë¿çtî>Œ'°¿Öµt@™£*¿æu9½æÕâ¿Ùè<œh¿æ'Z«GA¿ä)~HÛ;%AGNbcu3FGL J2200.9-2412NVSS J220036-241428?ïÞ_"WO"?h»¹‹hØ?0" ò£7?%˜ØE¿6p?o×Š^·á?hG]%$?ï°ÎXt?ŽwôÙp¢?&í\›÷y??F°÷'aX?}ð-îæ8?~—NЄœ³?ï?õ…Ó1?yâoA»?dÁ!uÏZz?Q¿¯>?•i+ßâË?vþ¸¹Æ ?ï¿3¾l‹?d"\O·rö?@ßüê켓?0"{oœ†?~J!,\âý?dõ&ƚo4FGL J2201.0-5907?îâD'oÀGW}|,¡IÀ;:p>V}À<ñ8Ë@ ¥xJŸ?ýs¸ÿnx?Ô—ç—S?Üþ#[ú§¦@gGzÕ@:ԈØ׿ëU ÃÄæN?í®ðBóš—?}Ö¨¿âGò½¢7x¿éØb,E¿ºRÅʤÿAGNbcuSUMSS J220107-590639?ï\–ÍYS…?‹¿+g°Á?€SVí?š×?}2ü©,U‹?ˆ†õ¼kƒÐ?'Ü[§€À?îŒð;ãʓ?¡YÂ?[k?sòâP¯-I?'yn–Ú?¤²Ÿ÷­q(?Õh£8d?ë.V«û˜?¢®×>?§óÏ0pñß?"¤Rz/k?º"cêÆÑ?š±WÉÑw?B"??'ð*Å5?ƒP	öAà?€T…WVŠ×?£ ~Fwí?šŒ¡˜À4FGL J2201.5-8339?ïäÝüÀ?¶,ºs-õÀ8¨á¼©iÀ;j¥P‡@ž«"‡@î.|M•?¨ß T« ?Âü]CÆS@ï»@ãÑ C—Y?ïGòrxÃ`¿å&H.ÿæ]8TÛ#¨¿ç÷#b…±/¿ëãIEÄ/o¿ïþâ=ø3-AGNfsrq3FGL J2202.4-8339PKS 2155-83?ïÐ+§']??pà…¾Å#0?d¸<º¸T§?cÒlã‰+?kêlµ?f ä"eÂ?k"AÑ?ŠÉ'²`_?JŠ¹µ$lî?[ªÐÜÐtÅ?ˆî¹œDÆ?š/~&C?í´ŠA"ïç?Ÿ WNòˆ3?¡…þ½ÓLÖ?•§á•`?£1])Ý´Ä?"ImŒ¡r?ï'!ûØ?"4¦¨' ?q;ĚOø?b3ŒÒ^|?–ÌìÚ¨ò?'ı¾OVI4FGL J2201.5+2950¿ìۀ¸]eGÀ4ë9Ÿ]ÿÀ;×gZ'À<ˆ~aßï@@)iÛ»Ó@^ø³Û?Ï7‰I`œ?¶¼¬™%«`?ç¬ÄÉ$¢@k—ˆrTÜ?ӇŒü¨1¸?ïë뫵%¿æ⤥fVv¿×–£EG¿êaQžÙ•?¤,٧ѕ´AGNbcuRX J2201.3+2949?î¸3hÜì?˜ãß«?lÈúË¿jm?dí$V»?¢²}¶:›?—'Í€®¼Ô?ïDњêA?'û_ÿ& ?R䐉-¦?bÀª"8j?–PüË
$÷?'CÉô÷5a?í©Žá~ƒ?• ªb!]?S¬8»¾M?w†0P̤?°Œ¾ܔ?'«— õ?jg¸?ŽÝœß™?~…¿Ù¡¿?k²8`~n?«¤ì…¾PC?Xy†Pb84FGL J2201.8+5048¿îᢃ'ß*Àdg`ai§À7²š²žM^À;L(Ê#¥!@¶Ý®òFY@€_†xT¥?›öAô?Â4J@Qü£T-@ ·áXJ¿Ôy!Ôæø¿ãyk@Àºp¿èÊ÷uR¿éñ‹@;¿ì¥2Ÿ9–¥¿ïÿ»!(ĚAGNfsrq3FGL J2201.7+5047NRAO 676?ï›Éw3Ï?~!âY›Êû?v^ Í?X?sÁB­šç?{½ <˜Ù?rüÇÐbÉ?ìõ耖&?Á֍˜?X½;Ü+8?r…î#¸Ó¨?·íÇÔ~$?ÁÉAœ?íšW(°f?ž;}ÆB?¢kœH³;Ó?–¥²Ô;å?£îñ5¡½Ñ?'¬Æ;y~k?ïÞÆw
O?d"æ`¬:E?BâÏÙÝò?@SAŠØ?l€Ôÿƒ4?bà&Ɗüx4FGL J2201.9-1706?êð§5A3ÀHØ#|ÜÊqÀ;Í¥,tÓÀ<Òï ´«n@$/ÿ¨Â+‰?ö…6+‡?à«úYÍÑ°?–´3<²&È?¬ÊÎþÙº?þ¶ìM›"F?çøäb•¡g?ÝYŽÏ[¿å>^‡tÔ¿ïÿZS2¬û?ïþSW•é¿Îîì\_&AGNbllRBS 1813?·]ú?Ž®Åa‰7f?+Ÿñ¿D{"?>wÝCrÂ@?‡-œË+oÉ?ŽrÃ6VÞð?îüèg±[]?­òH'?f™*fça£?‰mĕ¥?Í¼÷¨?©ÛQ/9Úü?ìiâ}{‡'?¢ˆ5—~ÉÎ?'^²E•Ð?~u&£³˜Ò?ºeËq!8?¡óÅ_iz?ëMœ.ð?¼A<9DÎî?3dB˜¿?Mz–o?¿Ý"óœs?¼GOý-á4FGL J2202.7+4216¿³r°Çi©À$ãb¥ç…¶À61â§)¥À:¤Nér@¸¨§ÿc@%@FA,ñ?"•1f:­·?®Õ¬€?T@$YH¾H¦@ UšSÓ¼«¿Ä¿('!-¿ÞýÀà…f\¿ãӉX=¿âÐíޕL-¿æ;a3v¥¿å(ê¥$èAGNBLL3FGL J2202.7+4217BL Lac?ìK,®Á|ê?®d/¶"Æ£?aï‡8"Ú:?_>i#å>?½P3Ú?®!ö*ºÞ{?ïã™.w?§ ÏDjgô?aÓྲྀòf?x{iù¥'"?šI†Ó?§.jM;	ß?í…3ÝÉ&;?¢êÙ$Ôlò?ŒÁNޟ»?‰ÏpÈÂ?°DhçÚú4?¡k w»§ì?ï¢ÌSAØ«?z
aܹì?S}]0â´?QšÔžÜ&Û?"Ý?#¸Ñ?xóB᡺(4FGL J2202.7-5637¿î'ÃH¶õlÀHÓþuóÀ;WçS`Ð$À<ג:)Çz@ —½çו(?üì*EMçê?˯ >#|?²t\É.²›?è|îh(?ûÊòìq-?Ú¡Ü>ñ§?îÌ Ÿ²¸O¿âsÞ-è¿Ï¤Váä-¿ïÿò~#¿?ïÿ·ÀÌ
ŠAGNbllMS 2159.5-5649?ï⾜­›'?eRã©ËF¢??FýF‰á?Dg«8F¹?iXƒ©"š?cRúÆ7?îÐé²°eÖ?žKTAV¢?e¹lsë>ñ?sj–Œ=ÞÖ?¡•Î
ºî¤?›è›_Ëuœ?íïB–‡ì?•îÐ9»0p?Œ2?ô¾$î?ƒ=Ì@ÆDw?°
=ì³ü?'ð¨ÔKñÞ?í:iîpD?T$l+?ŽTÂ|¶Äi?…	è暞¬?²e<`õ¥V?›.åÑã°4FGL J2203.4+1725?l‡	AÀ=£µ¿j
»À8:²ái<À;§I׺f™@•äô¶Ë¯@ÚŸb0w?œý( Ëß?³"a†q@ö_½Õ¹@ebÉ"ô!¿¾¡O›s¹`¿ß:ÆF¡¿åK~îóhB¿å7_ÞO¿æ¡!þ'|r¿érR,ó~AGNfsrq3FGL J2203.4+1725PKS 2201+171?ïÑã"`Ô0?kwŽø/²Œ?>õŒ±»ì?5ž;þxð†?uå";{?jsÑh£¸?ïÆRHö§.?€h¬µÉ1?0®IÛYÝý?A5@Þ¦Õ?{ËöæöËØ?€žüAÜP?ïNžP\5?Xæäsÿ?pÊPœ‡?k/£ÃPo?'ù«nw€?~¢±—|µ?ïúeæÞ-Õ?6†òö¬õv?
S¢Œ€Å?™Š±è4'?DwMäL?5wÕ:HÊ4FGL J2203.6+6751?ш8U(rÝ@#ç@š$À:[¤ˆ
%À;ÚVų-@å‹
µ'@—Ö›'§æ?Ï"¸ß/%?Ç¥ÚZ)O?ù Äeõþ@5àŽ5?íõ«gᑿèÿ|'1ž¿èсèM¿é¾x`¹Ô"¿ïö¡÷6-¿êÐØËЯAGNbcuLQAC 330+067?çî4èå`?Âó¾	ú
?¢Ì͖†>?ža]¬"fi?Ï
ƺå/?ÂÖÖóyÍ	?áø¾éTJ?ÌTè;öØb?¯w"ñ×ý?®ô­½5ƒC?Ø Ðol?Ëlh©®¤?äN¼…JÂ?¯'2Óµ½?³µÈaeâ?V&šyÒy?ÒvŒ"Ý?ª^-™ßV÷?â–L1ŒrÁ?¦ùÆ©	yÚ?·ë΢Fsj?œteC©h?ÔØsôU}¥?§?ap¼tÄ4FGL J2204.3+0438¿Ñ°ÃáZ'7ÀCT!BoçÀ:
,·îïÀ<Qé{Y<²@ÖIGF»{@­|ÀDÿ?»"žñ-?¿ÆÕfú5?þ`Î\‹@Íêæßó¿ãӕ:a%¿âôÇÝÏ©v¿ãiÇåv¿çôÓ˜A¿æZ1¿•¬¥¿ænnD—àAGNbll3FGL J2204.4+04394C +04.77?î>J' 2?¦h…|)Ê?kÑXó®?erñd©?ª^GöÄÒ?¥øËÑ-?î×"?¡?œUB?_‰Ç
ïûÎ?iaù«N`¹?¡'ÖWÈ,? fåïÑ?îÖ0cÀ1?ŒýñRuà?pãåe91s?a蝵? €}XV°?Šž\"Ñ?îÐ߃·
?ƒþ´6­'ò?xë뗀Â?dLT?Ÿ©£>mf?'D
~ßh4FGL J2204.5+3634?Í9\ÇEHÀ.\ÌîZ¼À; È1\™^À<J'Œ"Þ!@ <7"À@§äRµ?ÅÑY¹Ú¬´¿£§àYF˜?â"Jb#á‡@+
s†	š¿ç|'ݽµÙ?ï·õÿËþ¿èÉ[]ô§Ý¿ås]û]Ùпãõ
}ìêÏ¿œkÊÃ!?AGNbllMG3 J220423+3632?ï1‡ÂgV@?M –î,?\Xeö"?W´Ò»Ý–î?˜	‡lµÎÑ?âò Fn?ïk|<X+±?ß	ßû%?AdžÀ
î"?P>¡Î]Z?'<>ú2"?wəŠÅ‰?íhcúÜö'?–±n²qd§?}ë:Õcu?m%‹¼?ƒ?²Þ,{Â#?•Yü­ÕÕ?î
Ã	ۗÕ?'…!>í?j‡"®"LÉ?_ÉZ‡@?­{]7]=ì?''|¬4FGL J2205.0+7432?çî0Ïå@.dvò¥¤jÀ:å*Óa,À<ap9N@xs²Ì›@ùš‹1!?ßš"Ñ
Ÿ?è…ë1;â.@l Ÿ²¸O@¢ÊšÃe¿ï}Ë<©Ôz?ïÿ÷œ"/¥¿ÎI‡9£¿é1ÿŒ<¹Å¿ìËÃAe%?܂›üu¼AGNbcuS5 2205+74?æH³Ç­?Ê//¾'?ÒͳÖ5û?Ê7²ñöÂ>?""QÕZ?ãô*A?äÜÆ«¥?ÐYÊÞgO?ÐÖWù†ø?ÎFzÜTïr?¿¡ÅÁä†õ?¶WÇÈM…þ?è¬M®õ'?¦×\¯Zpµ?¶<(ÌýJ??_½—êü?Â0·–]«?¡å@€¾a?ã[Ò4ái	?½¿SŒ?Ñc2åÚH?ÀŒ?¹u(x?¿"¢ÁŒ>"?·Ù…6¸=Ñ4FGL J2206.8-0032¿ïH3®`ْÀE4Áü28À9Lå".(1À<ºß%•@r=Ô¡ØW@?› 'W?±g¨A
wž?³¯—‡Æˆe@šfH3u@c,°ã?ßüÒ¹u×ó¿ÜÛëc:âÕ¿äa~õÿK¿àA¨a2Ÿå¿í'C¿rq7?·ð©Jç…AGNbll3FGL J2206.9-0031PMN J2206-0031?ïÀƒ	`ÒÌ?tHú ‹?F!jD}`?><)¤®?|úNê>?ss¯C?ï¨F*
åÜ?…ðµ*ãn'?8 Áén Q?Jü6Âɬ?…-omû ?…%Úßáý?îyf¬H—?"Þðº‰?õ.™>%?ŠӕÁÿ? ¦—ïÐ?Ú?‡hªî
‹?ï²ÿå(M?kIÏè?(?UgÐÐÁÛx?F,†¶\hp?€"›Ô'Î?iw¼óõ†4FGL J2207.0+3607?¸+ßç¸À/°ÿŸ‡ðÀ;i£ÙŽÀ<c…Ò<xV@ 3
ž¤@IsÙìp?ɪ+¢› ?ž(Û@'üõ?Ö¡sÕB<@úm‡	¿ï¨P!ӏ?ëU°€æÅF¿â`‰ãC0׿éò"ý[
¿´t×~'¾D¿è '+"ØAGNbcu1RXS J220708.5+360935?ï¦~¡Å?"w¯v6 ?Tá-"]ßã?RiõCˆZ?œ=R~~?"gë¹(à?ïi]e(xW?•?"´‰B@?Dà'PùÄâ?_›b€.GT?'-R i&ì?"†°,ë?íI¡/a¾ë?—üzøÿr˜?~Ã
x»-?má©F¾x?³ÆÅãú|ú?–¦'TÏu ?îVSՖ]?CIÍ*ô?WÊÈÍH[?T"íC´f?§LD|<Yk?N`Àâ4FGL J2207.1+4316?펙•Š7ÉÀ$FÎô©‹À:"qDúÀ<	Ÿ)üRÌ@ ¡™Ê–çŽ?ûèQÃA2Ð?ǯI™§"?ÐÐÉ<qu@v.	þ†ƒ@	n(Ãm¨¿ï²¾™-c?ç'!þW‰T¿áeHŽå
±¿Ù¤þývŽ¿Ó-eÿ8Yä¿ïÿäë8AGNbcu87GB 220504.7+430144?î'ñ)¾®î?§¿|h`v?fb»®¬Æ­?d§]Á*y?¬Á©*D®?§XÜ"ª?î¬Æ=s"?¯¨9¤Ð»?H
*(h?XÍ+ön‹?¤Óg€&õ?¯…h¨Û‡	?é+#ڍZÌ?¬É@}µÌ?¤$h=8h?"Ë…"þë?ÆJV†|"9?¨o~ÆéV"?í¤ó0êѺ?€‰Y~?uÀ¬?eY9ìWŽ?±|[¯×ÐÍ?R'&§"4FGL J2207.5-5346?éê½ÑÀHóþ®û+À9yÝ÷vÅÀ<j'¨
У@oPk'kT@P.Ë?«¢•Ûc?žù
¦z ?íã™BÞç@§¶š0m[¿Ú˜Ïö¿â[ýÂ8T¿æ¼ìOIo¿å—,×Ï_¿êú³fÊ9¿ÎƘ*XÄAGNfsrq3FGL J2207.8-5345PKS 2204-54?ïÐÞâ²¥?t©élBY?AÜ)KrZ?8~HtƒEO?uU	†P¿ƒ?sû<AQ‡?ïËÚó3'j?€L¡ÚP]i?.½®%Lf¿?LBünã?y˜õAçì?~ڂFcW?ï3Hƨ¼?ŽëÌ­‰?iæ¶yË?b`Ñwe?–Z[Äæ*?€[¾öì?ïôª)AŠN?Eä·ÉÌ_?6ãôRo?,üN}$'\?Pòç\nM?AÀÎxõÝ4FGL J2207.6+0053?ÕŽ]ëÀD×ú~¶¿DÀ:±Öv™ºQÀ<Uq€Ø@æ«͏À@ÂCÜ΢?ÄàĦbªÅ?¢ñ·¤ã–?ÝeêÕÌP@â«¡.
"?ïîÎ_¢¿ç0Èè#¿æfA¬Ž¿ê}ÅB"пÊX‰m~¿ïÿwD;ÏAGNbcuPMN J2207+0052?ïf]´ÊÓö?£ ‡§Ya?P,z³;±?Oà,ëâ$¦?'2ƞúM'?¢õÝ&pøÏ?ïlô͛Y?')Y¾-?C¯[¼Ôue?Y",Qh·:?'Ãën§q?TbW#6=?î˜
£Ë
??œæå?l$,ɞp?\6šÁœó§?¤¼âöµ?ŒÔ}CnJ?ïwämµ:¢?uŒ\"ƒ?BƒLááî&?9³ŒQ—|²?oWâIœ4?t̊?ü»4FGL J2208.1-4507?ߒ'+·ýÀJ|ÁÁÖυÀ;É7PÏ%mÀ<òrâu«~@!ï0ì\?ü"þ_
?ßÓp?ƒ"µ?ªW[AÖJ`?ù²v‡›À:¿ïÿæ4|ßO?ïüv¨ÓÉ@¿ÐeºD	Y¿Ú::c~)§¿Ü˜bŒè¿ïïM•µ‹AGNbcuPMN J2208-4509?ïáÛ𰒣?…Õ¡cµ«F?ÏFð×?%,¾Ý¹s?mchÕ5ÚC?…½6¿å2?ï‡72š"¥?ŒÂüSGòÑ?>±~âU?PM·ÿÃh?<§iKÄn?‹Ò8ëJ"j?îf-;Ø?'zZ¨ªVº?tâl£Mæ?k?Äډîd?¬ö@à×ØÄ?û
ÈBa?îüÕ0q0µ?‹	J(f?K;Äê®ù?LCý<'?ŸŒè²"Ô?‹.Ù»ÚH®4FGL J2208.2+0350¿Óˆ–%Š—ãÀCõº² À;RӘ˜èšÀ<«ÏèàÿŠ@oŠD¼óf@ᇿ}?Ìb~dßӐ?¿¶œ´¬?òÞU‹Lϼ?í¥ð¼¸yü¿îÛ
F9 ?ïã>"¹…È¿à"ä0– Á¿ä!Fkõ ¿áz+ª¨µ–¿ïÿCaԆUAGNbllSDSS J220812.70+035304.6?ï®?úß&?"«V½£¨?P¼`ÔUè?MµÜW^Õ?'Xua‡L?"ŸvtÀc?ìbìðB ¢?¸&ÂCÅ»?"¦R=à? J¯ï{TY?¸$îé[²ð?´_·Äm*C?íôN'¤dš?î݉'?'ÜΓ¤æ?y«>7°-»?¬ä0В)?ŒÇÊúNl?èjk#	¼?ªðÝhà?¨«»Ãòñ?šÎøŠ\A?É{gbŒ\U?ªÁáê÷ãì4FGL J2209.4+4329?ïêuë‹÷À$h'­ÄÉÉÀ9ºÆîj¬À;›Wëy`>@˜%ä@|dý°šg?·¶ böð¿¨*£dÄ?ñ`ú@jµ§l@?än.¡©¡¿ènÓr'¿åHNöÞ¿é¼ÿ¿ã¡Ö^ÆßοÚÒÁÃÚ4êAGNbcuB3 2207+432?콙Ì^`¢?µû½8U?^8øqr?Y±BÈ /?¹›¼±+?´âípF?êŸ&~€Ë!?¯$÷"í.?atª÷{qï?oƒÝ¾«G?Å="Zå±?"ёKľ?êÖz6øæ4?¬Ê$©Ât¸?ejìç!p?€
{›äM;?¯ÀuMõ?ªo°YýuH?ì`T¬È'´?˜/oeÀ"Ý?€÷£~Íu?jˆuoSHö?ºü;¥K±?—ÔöÐyç4FGL J2209.7-0451?ã뵊ˆQÀFÅ£~õ©À:aµÁŒäÀ<JO¾"4®@ âóÀ×v?þD¸)§™?·V3M÷ž¿¤"4áÅ=ž?îRàw¤|@ÕºåÈú¿ì¯©Ggž¿Ø†d¾E s¿ÏöN»ÏÏa¿çȧ¤WÚ¿Ô³çƒ?´æÐÙ÷­¡AGNbll3FGL J2209.8-0450NVSS J220941-045111?î¾4ÇG ý?EÓÅÔ?`'!§H[?TÄ??£'qjx?œ¨+íÙÇÕ?ïLY¨ÑjÊ?'Ñ8ò"E9?Kµè-=ï?\ŸF2ù¤ý?•—¤iܹ?'
øb—¸´?í>?¢"@?—s–?ˆ'?'Ü›ü ?u¹ª|r8?³²pnéû?•¢ƒ¤©?í$1ÚC?›²Dê½?gY_P=Ë?`r}Å=ql?¶#¦3åKñ?›§b"*+4FGL J2209.8-5028?Ý,›úqö'ÀIƘÀ¤ À;Lï͂Õ2À<¤u‰ïØk@ÖÙyÙ_Ø@œ÷S½?ÐÉý·{W?±äØfÌh?ã´£
[£•@Úºch°?í«ñŠò6ê¿álÓu]¿æÂIá nu¿ßmA£¹X¿ë®Íb¿ï÷9R1%<AGNbcuPMN J2210-5030?ï³ê»Ç?'IÏéDQs?O{–-/Î?MUö_2ä.?bî:ð?påw€?ïŸA IT×?…"ÏŸ¢?9eâö®;?O
à"õGN?‡dˆÕõYu?"júӇÃ?îÛ³<0°Â?†çCL8³?mñ¬¨{ë<?iVH(\h? e±rm5'?"«ä9:,?ï{DæÀ¨¾?uBÔªlÃ?Nòê.•?@@JHÅIJ??ž^—-Ž?tà"'4FGL J2210.8+3203?ì'p Ú‰,À3Í_™Ã‹À;ÜjžÚK;À<ߧ[#<E@$œ^o÷à?÷&ª>,‹y?ѾÇüX€ ?ÂZ<¡ñ×É?ñÑU¡Îò@"ì3D{¿ïÿÿÊPË?æ´yï°&¤¿µ"¦:'ÌF?ïþŒÝôgp¿âüvÄ¿Ìp÷äÓ~ÃAGNbcu1RXS J221058.3+320327?ïòîÃö?š‹Ü'•ÑU??!xpà?A10¸zÇ-?ŽŠ7ÓuÁÂ?šg/Y
ѹ?ï`J¿N
£?ªP}‹Ò•?OSº;'z?{‹»÷{e?'ülÎü?©ëfŸÎ?íS¯ÖD‡?¢ëbKè?mʟ+s"?jYм?¶
‡ò?·?¢àìåö_?îÕS÷:Š? @§GD£•?pG¬;JO?söÕƎ }?¥âaËî?Ÿ'ô:µ4FGL J2211.0-0003?¤üßp/ÁMÀEy¥q"À:ÆîᵒÀ<tÌežÀ@ ZS6Ñù?ýP"{rg&?ÊXyÿ…V?»?äq"&Á?óÂíÖ1Ð]@Òì؅è?ïÕ1U¡Ï¿æŸÿ®—¿Ý‰9"ÛòZ¿ã^M"0ÉÌ¿ÂaÉɍ'E¿ç]Ä×5AGNbllRX J2211.1-0003?í I,Â|?¦kTHÚE?]Ÿ֐?X›uՙ-—?²ŠõPÐÈ?¦@"vý?îôˆ7;Ն?˜¨´†Yã?\u¸¾)?höqÿ5D?Ÿ§ŸGiÃ6?—d°&Lmg?í]ÂH·Ó6?™ƒdy± ?v¾ñ"ف_?g£Æ0ı™?³¥þ óÎ8?˜ÈÏòÙ-?ìp¨Z Ÿ?œÜš
?iäÙã0à½?a»"¾ûÖÏ?¿%Sît?œã¨š|4FGL J2211.2-1325?⟝1Ý%hÀIÌ>1"÷À:ŽŸj"óÀ<U¢šÊB@§"å¡ì@™f`‡)U?ºöÄBÃ<?¨æª"xu?ßÁ6+57ð@Ó1p:z¥¿ÄnÖ·Ý&Œ¿ã[	pÂ	û¿ê֛'§å¿ç‰âÂW}ë¿ïÿåþÌú?ïÿ}Ž¡AGNbcuPKS 2208-137?ïõãà'?TyG¿'ò?9?‡<}?8Û¿?KкzÆ?OÂÙ	Тg?ï¸[ÖS?†Ír'Á?4èË°ÝÄ0?S'>­ùuŠ?Aø,ô|ø?"¨ƒë·?ïKD	ò?veŸ*áä?i®4š™ç?Z¼¶à}Ö?"a¹x.\ì?tl	Ædß-?ïìò<>­?Q!j~Ì×?8¯àÿó1b?0~"‰RØî?_ïB©¨?Nâ;£«³á4FGL J2211.4-7040?Ú\®j͛ÀD~	VÀÖõÀ:÷Óc¿ÂùÀ<À!ˆæÃï@Šˆ¯'@¢P¨­?½¬/ô9xG¿¨•Ú¦‰¨?ìUÐììýÅ?þ•'¦8
Ž¿àr·B!À¿à-YÕ^kƿ剀Fâ<¡¿ã¿ÕØå	¿à­á¥!¿Û¡œ1úNAGNbll3FGL J2212.3-7039PMN J2211-7039?ï5].þoi?"ïÍÏjÔ?f,³ê¯ó?^R|Í2?–ŽÃ¢ÜW?ÛH[yÊ?ï<÷ÿ#Ç?"(8ÁeÝk?R¥Ð0ÌR-?]Cwƒ£;»?œîýÂ1?'z…ü9¶Q?íôž¢˜É?òq»–¶
?{)?iWîh }?­Pòèƒ?èzè1?îxÈw-Ê?Ž/Îî´ï¤?v-ê'o?h)OÛgÀŽ?¥­ÖŒ*±?Ž_Σܬ84FGL J2212.0+2356?ëçÄRˆlÀ:q£±JÀ96ÁU FÀ;㶇*@´¸­@óŠ§ß­?¬ç…›ñô¶?¸É»{Eq@Á _ò@Ó/m¬¿Åº™™n¦|¿Ý7zU0³ý¿âÉUÐ-¿ä×àŠ"(¿æQßp¾Y¿à—àýy½AGNfsrq3FGL J2212.0+2355PKS 2209+236?åœÚ¢¿$ ?Áè‡ê€Ÿ?•p»ü¦ç!?Œ.ZAëçd?Óo>ú·HP?Á"΄߃?é)å÷×#?Â~_LO<,?¶÷Àóš,?¼j'‰Gm
?¿¹2†í¬½?³·¯`tT?æÅñrMp?¯¶û߆?±xÜd˜?™ö¼"vó?Ì[}ș€t?«Ã«]8ß?èíö'óþÓ?¥mØï]?±
»0è?•Ÿääl'?ÃÁIҐ¥?¡õøiÁ+ø4FGL J2212.2-7251¿ïgŽð{Ü"ÀCËØà†8À:ùÊd<À{À<"+¯±3@ˆºÏa@¦T…"RX?Ðkcü(Úë?¶å¸åº/?é¢Nt@fãr«™ ¿çò/ýô¿æ\°ožôL¿ä–_'‹¿ç!·à¬~¿ìì¿B ¿ïÿA(¿;ëAGNbcuPMN J2211-7249?ïdÿ+çQ?'-óÈ`Ã?[òÑNtrÌ?U|6™ªs?' ín(ÎÏ?¢5ZÃ{Ž?kÄį?¤|X UÄÚ?^
þ>Ό;?n¾P*º-0?¤71Q½@À?£nÎ|ýþ?îφȃ¬?'E廿ì?¹r'øG?t-uߺÂÅ?ªTªî¹³~?‡Kv£Û?îä'9CT?‡Z•Nvè†?f!Ú6'†]?V<¬þ>µ? ]™I¢E?†µ¦¦ÀD4FGL J2212.6+2800¿î*0•Ÿ#À6ülü'œþÀ9ëÕYcH¥À<O'h˜p@™õ *­S@ãøÀpø?¶t·7_?³ÛÙÚý<+?üüYÒÚ-@X±G
V?ïäC '?à¡
+a­š¿áÑ0ߛÜj¿ã•"ÁËçÊ¿ßÛڜCB¿ådÏÝùDûAGNbll3FGL J2212.6+2801MG3 J221240+2759?îU,ÆÕ-¯?œÞÎxôÓ+?xœ³#¾N?pB{Жð€?§™.JÍM?›}eÁãá?îfm°?¢ãíxõ¾?{ÎV~{P—?‡É`1
?¦d0UÎ? &pÅÝTM?ìIbôï?Ÿ"p6³ g?•êœe4Z¢?"ç2¿ùC?¹£
ÕûAá?š'¼{þˆ£?ì[qض¯?™Ç¹ælہ?£9 @ÿ¥@?fOE¨?³‡¡Ê´Š?"b¡oD4FGL J2212.8+0647?êõtYe™ÀCfƒ#5.À9ÒÏr™zÀ;Ø£'@ßÄ@/1ÜF‡@m«w?¾fLæ¹Í?Ãx~‹ì@'pŽ@ÕO¨3æ?Ӝ=bá÷¿âS	AÈ!l¿ãܸ2¿êÊ©ÂÉn¿éö•žoû¿ïþ-͘¤§AGNfsrq1FGL J2212.9+0654TXS 2210+065?î¤ÿG[ÜÒ?¦³kk=Ù=?‹ÊOçì? #)ÅΈÜ?—±ìõñ¤?¯…Õ?íÔôj÷œ¯?²R
éXÙ?È<ÕO7?ˆ'%‡`?®·±Îk‹&?±NÂàhö?íßáê'T?šŒâ•³h?†©óßÐ4É?{×fâA?¬Wde–±
?—	Ö-£ZÈ?ëË
Õèú?—Z$i¸°?"ñëÕ£w)?}Oo'‹?¼kçÚc?•
XÿÇ4FGL J2212.9-2526?˖[îà•NÀKHßÞøH|À9Æ÷ê‡È·À<f1ØÀ @©þÁ'…@DAãÐ'?µ_ý–™4?ÀT5¡Íoµ@áDS@fý5uWÆ?ïeç}R;¿Èô 8Y¸®¿äövŸ´'¿âŸb2Ô¿éKòJ·¿ïÿõž}.)AGNfsrq3FGL J2213.1-2532PKS 2210-25?ïãtôfæ?e
éj¢Ç½?Dd`|¨­r?Ex:¦1Ê?grÚìnï7?aô©ž§4?￞Øt%?'›‹Èe?6ø¨jOöë?NÚ fߞd?~Á	?Zîj?‡…`'©†?ïþ)Hlæ?…B0Èpj3?vðàaÉf¿?pÖv`
è?™ä¾€	®?€¿Ñlã?＀:VSÃ?cèg¡©Ý?`…¿njU?N	ž"2)?y}Kè}?`Ð0ý ÞÉ4FGL J2213.5-4754¿é"ôTŒÀJƒ2a|ÚÀ;†¯²	ÓÀ<²§$œ—{@ ´-"¯¹?úèleƒè?Ð04:Å"ß?ÂîräÎ÷?ò"ÏÝù@'óƒðºé?ïû‹'™¿ìYÙ$Éã俵Ûc¾k`¿âc€4
¿ÃÇT}ZÉ¥¿æí¦a(9AGNbll3FGL J2213.6-4755SUMSS J221330-475426?î"ú˜ÀEX? @½^=€?W·¤m‹0ž?Q"TÏ0Yó?¦ò™PQ? /|«8(?ïG·c%³?"Сyýš?RÛKÿsæÌ?bdqO§dv?•ñtS¤G?"x7÷PM?íNc˜°%?–êЭâT<?pŸóeªêg?^á`†mú?´'ä%@.?– €\©1?íÑåšfdì?'À¨êá±?KHJ¹I˜?EÄ^³9X?±:B—Yž?'«iéê³!4FGL J2213.9+5948c¿é¸a\€"i@½ZiÀ:ôÏJVÀ;N[`xæœ@É"
–ÜÑ@l¥³Û?еHŸ¸?ÀNL(Í~£?ö'SZ(@GMƒA?í#Ýàpm¦¿æ͕ŸŽü¿éÕÀ˜áä¿å|ßÿÚkF¿ä9AG`¿ïùÅôkwGAGNbcu1FGL J2214.5+5949TXS 2212+5958?ã1þš=Æ?ÃrÒt)ÄÑ?‹tvP…˜ý?"¢ƒ¾¡Å?ØÂRPGW­?Ãsž¢'¾?Ô/ /‡™?Æ6û{ƒÉ%?§(^EŽPW?¶aª:Ñ?äuê&×.?ÆEÊ·è«ö?Þâ;sLL±?³¥…aò™?¨@ŠùKKû?'¤|qZe™?Þ³-ŠIÏ?²&k†cÜ?ÔâѼ¾Q'?­•ñ_AV€?"b¿¬Åš½?ƒÌ~ϸ`Ë?äë$:ªa?®y_lu4t4FGL J2215.4+0544?á×~4Ês<ÀCý—€º¥ƒÀ:¯¬kbOÀ<ióB'[@^´¸ƒê†@†ƒd£î‡?Ärj@:­¦?´Eyܺր?ðé›9¬Éø@ár¤P¿ï«.ýn€;?ïÌÄ¿77û¿èê~eᆿԑMjÙ¿çÂ[úҙ•¿ÈNÕ:¯~]AGNbcuNVSS J221513+054454?ï[V_Ääê?Œ
–ìC'f?V‹N—û©?LlSt'di?",iã?‹^fX×4B?ïb(¤(	™?OØ	¸¦r?GÜ]>Cl?UΎ‡-v?'ü'±?vãÐRe?íÔ/ˆ"þ?•Æ÷Ò£?x#6=?dÆ`†¤)º?¯¼8¥¬)O?"uëu¬ t?î†þ!{?†´°‡"?obvw?n²ÌÑÚö?£Z*ÄEJ¥?ƒÓ+ΤrÝ4FGL J2215.4+6105¿®7Ðf_Z"@
ª:›À9æ†t"çŒÀ;edù~Ü@GK1¬ ]@øÍ ¯¢ð?ÌèæˆàŽÌ?Îü¿¿s@Õd¶býü@y-Å
5¹?îFÉ))?šg8ÚxBB¿çÄô'6ô‰¿æºÊ×)G!¿ï'>ˆPò¿ïíx:¤AAGNbcuNVSS J221507+610506?µ°Öh 
h?©¥RÑËÁ?¹jƒ|8?²xØåh¹??ê"ÐL}Ì?¸àÎs]?ýðHô
?¸œ\¡Â;?Æ8¯róúÝ?½D¦Í$?層§0ÄF?Á;ò@ì—Ê?Î
›)õÕ°?«LyT¦»?Á	¥¶q"?¡u
0vûå?ä;Ìî3?­ÙìÉw«	?ÿ¿a`Ì?›E·Âl»)?É
3° ‰?¨Ék"–
&?ä͋Ïß«?©2ÖÜ«B'4FGL J2216.8+3103?ïûw%Œ'±À5Cú*ÓéÀ:'S"¾À<6­•Ïà~@êûRò\@¼¾´ .?Ê\#—^ÖÐ?Ìvh&¯í?þrÉä»@ÅR¥>hq¿­QƒD1w
¿Ùè:œ3&ô¿èï^&üĿ拃ŒÚ¿ïýŒÙT›¿ðAGNfsrqS3 2214+30?ï'Þ#'M?…·²¢â«?zíðó
?€rج*x?{£æFfhq?u&â<,'?íòߝbˆ?¥µìßúÿù?ƒ—Z·±w?ŠN°{"Í?«ì7h=y¡?¢ŠA÷²0/?ëhdñ#p¼?¢ñ†ƒRý?¤ÙD¶X|y?'х®?ºP6¸;ç?›œM³"šG?ë¹<©Šº?˜WŽ+?£ ¡Ï|E?‰éo´½4?¸¥Î'õ‡©?•PvœM`4FGL J2216.9+2421¿ÐÒZ?ÜÀ:r¥'ÛçóÀ9†B"ÏÞÀ<*4žm>@oâ~9ì¶@é©¿Š¯?²˜;J®Ïâ?¬uüº?ø·…Ýúòz@
°ÕöA:¿Ò}ÆUˏ¿á>Ÿ&Kn¿å–¢='¿ãh4çÌ-¿ãîª!üÿð¿ì…ΫÊÆAGNbll3FGL J2217.0+2421B2 2214+24B?ï—aÊÔ/˜?M(",^?G¿UÈr*?>Ì­ˆ?ˆ«—îlùë?~‰üˋÚ!?ï¼Oèµ?€×SJÇ»/?2`è¥×è?C·sÕ)×k?€Xþ¸åd?€NÝ:Ø4¢?ï5¼©ªej?{þϺ+ƒ?i$\£ÁÛl?SÚ×sp3?–#ß6;s?y½×šûu¸?ïÊ'ÔF?p¾|U`ӟ?`!òۚÒ?I8´š5!ƒ?ˆ0Î7"?n¸–Àñjm4FGL J2218.6+1941?Ù<®É£ïÖÀ>P;€AÀ:ß!5Ú­`À<L½}®'@˜o¢û@V	™Üµx?Î
	}Ø
?¶$ø¡«¥¥?âÙ`>.8ø@´4¥y!¿Íg³BW¿Û•=׿és¹jð8ã¿ám —d¶¿ïÿÚpú>?æÓó! 8ÅAGNbcuGALEXASC J221854.64+193841.6?ï†cž$Òê?•Ȍœú|?Vo¢ÂÐ,¾?NƒuBÊÓ?‹™$q@?"ënI:/?îþ"'¾1j?£C&•µs?Y…>QÄ%ý?i'â÷U`Š?ž•'#M?¢¾‰ÒÄç?í".Fº?–ýòƒ²?‡Ú¦ @?w–øŸËBÙ?°|>;8ö(?"~Ž¡J?ïTMk~?'Fl÷RK¡?b,þXw?R†×†'?šÁвÅ<í? ›SJ4FGL J2219.2+1806¿ãr"'¿RÀ?¢i'ÄÀ8þÏ;<1À;×Q!ZÛ@¢ª‰Uÿ'@l@šú©?©¦"Ô¸Ôr?µh¯‰â@
¾cb¥ç†@"Êb9[¿Î"¤)•z¦¿Ýˬ;\Í`¿ãü& ûù
¿ã@/€ Kпè|·áƒ=7¿ìbíç$AGNfsrq3FGL J2219.2+1806MG1 J221916+1806?ïÀÁæÁ˜¾?t"ž‰«Ý?<ñ¤¶*Ö?5òD#¬'?}ÏòSÐô?swVصÿ?ïП¦áP?zx/þ_Ñà?&­œ˜ºAn?@[%Í þ?vú¿ª¬†€?yÆHy¿ÂÊ?ï!"Ôàê?€%&Ÿw?r²_'?a<ã@Ÿñ_?—MxÛJã?{œ¡8?ïòýeü¯?G(œü1˜?rϦÂ÷?ڏ	óÖ%?XÎùš'Æ?Fœ','©r4FGL J2219.2-0342¿è®ËÆx°ýÀGfá`؇ìÀ9Ê©Hš¤À<*yØ32\@蹃ÄÆ@ôɅðoi?»Ë"?À. ý;)¢?ü6öl‡š@íèQ¸"k¿ÏX"¿åޗ¿æ·û"p=¿è§:¬Î*¿éÉc@—ë¿ë³@S'D¿íý}¿HÌAGNfsrqPKS 2216-03?ïÞڔc!À?}¦õgá?Ca8`1?Pà%±×m?la%D)Ê?yÃh¾ã½?ï°¼A‡?‡ÉýÓúaà?2·ë¤³yð?K¯f¿?ƒ;0AÜá?†øË?t?ï5«,(M¡?~J³5蕰?míTÌ8I—?]M­1AöW?•ŒïáoB«?{•ý	•?ïÌŖGÏ?bßnÕ»í?H¦ƀEZ?6íÿŸ¹p?v"à#
?aaGˆýs4FGL J2220.5+2813?Úg»—žGÀ7ÝÀµgÀ:Dmî$À<z8Cƒã@ ÷X¼…?ÿ
ä)à¤?ÂÁòh½®¢?¥Ø£š¤\?ã¹
"BË?þ'ÒÐÇÙ?ïú{üР—¿è¬Ôÿ÷«¿ßd­ÿ'+¿¿ÜÆOo©Ü¿Øå$ýd¿æÄç=AGNbll3FGL J2220.3+2812RX J2220.4+2814?îìëÚÚ?•V^ÀˆÊ?Wîk·Ìî?Lz‹Ÿz? qÏšCó?"ÿ-ŠÌn?ï']
"¦
?")ò±jË?V‰%ûtû¼?nÅR"ff??™«Ëûóî¹?"£Æl.?í¹ 'òÅu?"Îk±­M?tá¯^â)?^øð{m$?°äàr{´_?'7ڎi®?ìæB2‰¶?'.ÈO'åÔ?~¯"d±d˜?jI|?⅖?¶âýH œ?Ù"£ïcm4FGL J2221.5-5225?ß8çJ°ÀJ1	á*QãÀ9vvü¶ŸdÀ;ñžbeP@üDËaé?ù½R;66ô?°«¶ý'¢1?ºˆ©t
n@‹"ÞQZ@Öjˆ	#j?Ö\_ý@²ù?ËÙÂ~•1U¿Ó¹Ššù*¿Ó«<äâÃ.¿Þ Ý%	¤Ä¿ßÝD>HeAGNbll3FGL J2221.6-5225PMN J2221-5224?ïÔð¶|f?k¸ÛñšÙ
?Pmê'‡?G © HŠ°?q€	Ggk"?hàhR=
?ZÈ?Š'h¼¯3?@dú>©?S¨ž8Ò«?†—ÙÖþº1?‰]³è"?îúó†ÃEœ?…o'|Åq??uuF5Môâ?r)æÚG?›D=šCÏ&?'Q[ŸØ€r?î×n"bt/?ˆŒ‹Ü1ý?^Y˜<?N>´ˆ–?¡–Qܳ?ˆl<Íf£4FGL J2221.9-3504¿ïÁ£n.±ÄÀLžÁ~ºñÀ:ÆùáØ͌À<§¾Ê«Š]@û±r(f|@}õÏ$•á?ÉìtÝÍ{?Î3†V¤?÷E¶ù%ñ+@­ÇÜMj?ïþ[Ï߿⿛L4¿çîYyîÙg¿ìîiÀ
 пøÌ?îÛ@Î&i AGNfsrq3FGL J2222.3-3500NVSS J222227-350942?ïÙö½Ä+?u6ŠJÎÚ?DÊFkûí?Pó8Øê…(?pkX]¼õñ?sу°Q:æ?ïUÇ-°Ã?›uͳD1?a¨íÛ3?xÚÃ/>Ñr?"$‡|©l*?—7ÐñÌ ?îK¯.\'Þ?'™q:î?'¡žšÁ/?xo÷•I¥«?¦Ã$²!à?zñÝ×l?ïÆþÕ÷|ç?f°«yÆgß?KäsCÃ?@2éÇî¢k?yãs#ó?dóO]ãØC4FGL J2222.8+1209?ï¾îÕW­2ÀBWìÝ
Œ°À:c5*"8	À<8wškP±@¤ÔpZ0"@/MzÝð?ǜ
b.žN?Ł柆Ã?ü!¦ä÷·@T?b¿â½/k'–G¿áÎ耇yÜ¿åƒ) b`¿âя–n¿ïõ´yÒª¿ï}lÝxì{AGNbcuTXS 2220+119?ïÚƒƒŠM?oà¼À&0?M" âÁH?MwÇ´†5Ð?n™"CÅj/?k­i)¶ü%?ïuèoù%?Ž´8)»?Jy0‹QU?_Ò0§ðà¡?o&<?‹àJ¬¥t%?q|S?|³§ßý?~͐×$'?tøôpûÉ?£75íVM?Šçy@âí¬?îí¬']&ƒ?'ûö ´B}?p	6îh?añ*爨?žH)柕ª?'.d€¢Hû4FGL J2223.0+6746¿íÔ\B@!©Õ<ÝÖàÀ:~?Àà/€À;Ú@@aïß@dða|qÁ@K³ŸÕý?ÊÜøHр?½û
wÓ N?ò_V§¬Ô?ö"hëPñ_?ïî}†¸–¿ç6geiç$¿åý·³àm¿å  †Þ+¿ð?ïÿÿ)@k*AGNbcuTXS 2221+675?藮üÝZc?ÀƒU*NXæ?bX˜ÝQ?¢¬Tjž"é?Ë«‹Q ?À'Øè½?Ւfqm?Ëˤ׆?²ÌÉúÚ?¸òGE0\?âÝX
¾·?ÌIö£;†
?äæéÐT=7?¬RAvé³?­{åÞ*ü?•n'ZŸ?Ҏ¼â›À2?©ž6ßÇ¿?ÖsؤÜuå?±í²3í¾»?±·W²áš0?œÓ"Ìïà?â(·5'È?²6¡Ž"!4FGL J2223.3+0102¿çW1õÆk4ÀFMa€M˜9À;>Õ'åÀ<‹wI¹L@ Äkq=/?ü›Þ'׶5?Ñb
-€l?¿¶«G—?ñÞâ^.‰€@é£È¸?çÃ_›q
.¿çXÛch…%¿ãØMꣿÇÍ×0¨ê¿Ý·R<7馿Þ4hݏÖAGNbll3FGL J2223.3+0103SDSS J222329.56+010226.6?ï9/8Ðy	?ƒÁZøp&?C"Ì·›A?5Xº¤ñ'Ú?˜=ò€8J1?;ʎw¹?ï7¹®VŸm?"c¸žÌ??P¯&™–1?`•ÏÑ64Œ?—ýײI?"TF6ÎA•?î¾W+W?|¸ì;7?laš!‹¢?T_XÒôž?­xŠx{ñÌ?Žšý•¹?íG·i)?•*A.»âê?^컵î)?Q2©Ø4T ?µJ£ßUÞþ?•?ƒö•4FGL J2223.4+5814¿æhO(v®?軈!!7ÞÀ9ƒÝòŽþ5À;'éÃ}˜²@ºµ ¶Cs@Ù¶3kg?ÌÜ9|Mƒl?Õâ‹ûÌ>²@é!S6ß?éðŽîoß·?ïûøi2Ɂ¿ãç—¾Vè¿çðSà&ñ±¿ï6©	y&¿ð?ðAGNbcuSSTSL2 J222330.04+581350.9?êPO/¡¿2?Äʦ<‰åU?…ÚFxTJl?¢ÔÝWxô?ÅaÙó¾'?Ä'(àÁ´?Àœ–‹‡â?ƆÝ9ë
$?½»Öj~'?£.	¾9?è!~Í
\w?Êá›íª7?ÔG?Nl˜i?¯ VÞ2?Án~ËOŽ?¡ŠYÒ¡?á€À±Vßè?­YË0óÐÉ?§}òÏP?"ŠÛµèø?έQç7
­?¸Z²ò¾¸?æä3§K°?¹Mœdݚ4FGL J2224.0-1127?ï!h€ÀJ­>'À;X"üS£À<m
Ø/×^@¹¡"I¦<?ýœ>	P
Ú?Ô38üö¶*?ØÀyJ]@4…]¢r†@Fg˜jš¿ê6ñL¿ëk»À5Ö¿Ò\rœª›¿Û×£TY¿é4ց+Ž¤¿ïV›LøWAGNbll3FGL J2224.6-1122PKS 2221-116?îȵMLwi?š–~AŸÍÓ?m­˜Wí?jðÌ˜?¡™Ñ¥ÀŠ¨?™Ì‰¬G?îáÂëZà?Ÿ¡[Ú?d/DÎ䛼?pWå…\†L? ¬"\A?;&¥M?ìQ¢æ?¡¾ó¨
³?—húo¡Ü?ˆýýRñY?·˜°Ãò™É?žáJEŠA?ì®"œú»? T¡ž¤?r¦)`5?eԞmÍÒf?½è)J)T? #ޖ'!Ì4FGL J2224.3+7737¿àÁ¡ÕŸ¦›@1€¾×@ÄÀ:yôºQ À<Ó'¹¬@*CÜ΢@ˆE~R?Øb«{™Sy?ÜÓ¸#rué@ÊÊ¡yaì?ü¨pÄä &?â{à­Tb¿áʁ=­4¬¿é1G ¨"¿íè?÷g¿ãŽYÊv±¿ïÿÿ>¹úAGNbcuNVSS J222721+773319?è -"û"?Ã&q–ìí?´Ok«Mh?³è×è›ÆC?ÅW"ÞUŽ¾?¼í||¿ò?èŽ~›ý¿j?ÆAp2(`?µðëµÊ?»Á_zïÞ?ÂÍø'r?¼ôÎÒ7Ò?åkE‰ô†ø?­¿ü纗%?¾p™Zt?£7¥÷W4?ËO1‹€©Ú?¦u
Ú®ª?çªÜ+&@O?¬ú"[5?¡Úpûî[ç?•2ÿÖ_Î?ÌÝókgÉ?«ÂJ!÷îÕ4FGL J2224.5+0353?èÃðÁYãÀEriƒQX¸À;`P‹2ΉÀ<ž>xá"@ ËÕ§½?ýÞeæä¦?Ð#$< DY?Á>ڛÂhÆ?ó&eYöì[@'Ãfœ—%¿í²æ§ieõ¿îEÊ¿×Eø?ïÿë""i·¿æ
Yº†y+¿Ô7ü:ù{,¿â¯má"ê¶AGNbcu3FGL J2224.4+03511RXS J222426.5+035445?ït
¹ãEõ?‰K¡(BàM?Ab¼è?=L¿Í	t
?ö³'Z-?ˆÔHÃÇ6º?ï9ð˜^?"p9+´ãS?NÖNWôûl?_®6dÝ*?—åïz4–'?"gcÅó?íØK•iƒ—?'Ÿ
*#å†?qJ,ؐJ3?^;B8Ñçc?°)‡*Þ¢?'ò¾ÿ˾-?îu<¶;B?"WÃèfH?CèìaËd?DZ*i¬?¨\"T4Ÿ?">ñ݄ŠO4FGL J2225.5-1114?íº´'!ëÀJ"Ĥ	_$À:¨ÝÛ
À<OÐîš|î@ÌÁën ?÷@]Øù*ú?á°Þ1Î?â5~†mÃ@ïƒ9@ØS"¥å¿ï;Wú'ص?ïí%HzÿåŸ/ۏÞ/¿Ük®Œp¿ïÿÿ" 5•?ïæ0¡¢AGNbll3FGL J2224.6-1122PKS 2223-114?ïÈ^á°.?fŠʙ?hW–è¹7Á?u&@g€!Ô?o£
5–šì?qrÄé®Ï?ï.àʏø¬? OÅôD|Â?j­ßâŸ	¾?Š!8(²‡0?–Î*±­	_?˜r‰»–?맢—Í7
?¢ñîk!ø?£¿`E1èÈ?' "hº?¸ã;ýSK?ŸC¿"Ë:â?îþ<_ððÜ?'sÍ>û[?LìՇ
È?T¡Ì͔:?ŸQ
U©{¶?'E,ˆû4FGL J2225.6+2120?®ÀÓaÿ^À>ó^1
¿À:\‰mÒkÀ<.2$?zi@Œ9j.òÝ@4ä†&ö?ŝZ³Ê?ÑöJ>ès@"éèwM@	¸§áÛÒ¤¿Õê£	"¾¿ç˜¨"HK¿é¾Ðà­ªH¿îš¿^z4¿ïò$_°¿¦?ïw:ÿ°NèAGNfsrqPKS 2223+21?ïÕ¶`‹ëß?{Hm
?PÌÞÝ=W?R¡78ý4?pñ˜6ÒÁ?xj»ùYÚ?íd&¥?>N?´^DƒšÚ?çŒûªAw?šÏ1Yæ?±!Ù6Å[?¯ÿ
žCf8?ì«é5¥?Ÿ8–ÚN/?™"r©õq
?ŠŠ?³…"°öŽ?—¦¾Ay·?î³<f¬í$?‹úüg>$#?Ù;°í'?qãÚjùm? Uø†Dòn?ˆLÓ¿Žo¯4FGL J2225.7-0457¿çu!ÓörõÀHjœýÒ(VÀ9θ_WÀ<
¥T¸¾ù@š"ÀC§u@úÑÂÕÓ?«Fg~¥ˆ¡?´QVßµ²ª@—9~¦Ï@¦Mhky¿ÃöXak¿áâÈa®Û¿æÜrÒ¨"¿äØ`^'i¿êTCƒãNï¿ïÿÊñ*z'AGNfsrq3FGL J2225.8-04543C 446?ïÖÛì§?ihZÊy=t?@Ñ\WfäD?6<B?rãf~¿š-?h"ne
â?ïƎ îZ?€"®èò?3Â}uÆà?LG@¬
©µ?{‡S`û¡¤?i2^±÷é?ï.þ¼"³À?€­Æ­×J?n»¿¶[?b M%ß'?–Oñ',?~&à8<Š?ïè³×Â~?U¼‡Þ%^å?;€=¶«?0Q؟óÀ?cÜ(ŝ*Û?SìÃæã—4FGL J2226.5+6901c¿êÇЈ2õ@#mfŒ&À;L‰~™cÀ<FdÆ@"퉰ÃW?®ìc.è:?æÚU웟-?ïþÖ¿ê¼!@¤Œ;ã@¾i¼²"?è0Ì ?ïò솦wοØö™NðþÛ¿â?Ö¿¿É?´ß´°÷.¿ç|<[Ðá/AGNbcuNVSS J222625+690207 ?ÜöFqvó?Ìê+*í?¬³ë2趓?§_ه(>u?ßs<"1r=?Ì°w'Up?Úõ¯‰ms?Ð×7DÑRõ?–¼D¸ÿ	?«ÜcÃG»?áÏFN?Ð7¾0J
?èPEª'<?©UåÜþ…?§©Mî­m"?'}è˜5?ÈԘ}ª[­?¦þöÛ¾?ä@J#—?Ƈ8…"-Â?S¸çt'Y6?jŸˆX.¸F?×l"EDx?ƐYÿ•¡4FGL J2226.6+0210¿Ø@àÏ|ï.ÀF;€Ü3rÀ;Y.yÖÀ<…¦Ž@!¸IƯc?ûÓµõó?Ì^ív:™Ú?¶&	>˜7?ì%vå@ú5ÏÅ¥'¿ìÉW,6À¿ïÿóÖ&ã?ïÿꁺ¿à>"7Z	¿à	bŸ‡oK¿»'®îÀhAGNbcu2MASS J22263636+0210373?ï²ÔSfæH?€¶UQÑYU?$.…²Åw]?ó~©R)¢?'ú1{XI?€š5ÉSÔ^?ï[ª­EÌ?'HQυm?Eèöý™?T«Îg€¾ý?"Ûb¦ÔŽƒ?'•ä³ÆV?íÁÐ?…Fú?"a_P9"j?h@ÅÐN.N?TØ^DAðP?±/wÕSV¼?"/u'=ç&?íýr‰–à"?—Bgå–%ü?B~ז$"?BÓ¢µ(C?¯à¹k3ž-?—7çïTE4FGL J2226.8+0051¿ï®£Y5ü;ÀF°CécÜÀ:2lÙG."À;á/Ø4ßÜ@§¶¶@F€d?ÃßÉi@
‡?Îz°m¸@Œ:䜸@×æ\ÀË7?ïÈzW´ò»¿ÀÐâC5à¿éaJÓbé¿ç޻♽¬¿ïÿŸR@>´?ê1þ –
AGNfsrqPKS B2224+006?î‰ÉØ?¥ÿŽ–€5?"ª÷SG}?"E'9¦Å
?¤2 ¾Ê? Žî³²¿ù?ì0/V?·×"a¢§Õ?›ÓˆvCt0?¥ÎÇu@E?·†5XöÀ8?°·:Vê& ?ébù°¤ ?©"¦ ÏU?¬Î)@0_8?•¹µÍ?Ã@Žíagò?£=†á'?èKìåÖv•?©ôà<ÅöÚ?£"8߸?ëý{gö®?Éë~a.7¤?¨Ç4˜Ü|N4FGL J2227.9-3031?çˆv‡ÅÀMAð€0<À;n4˹§VÀ<ØYí²¢@ ò0´}Ì?ÿlº=~?ÊYÐ@tº<?i6+»W?¡±‹OÈâ@®©ÌĿ¯ÂÐË?èéÅ+Û¿¿Ö@£[å.¿èºÿƒ¿ÄõÊ\…!¿ÚÄ^Ô¡­dAGNrdg1FGL J2227.7-3036PKS 2225-308?ïÍUóý¾1?tºÀrZqò?2ÓCˆmØ?-L€/ü²?x'ÑÈ €X?tfZ£Ê¯?ïË'Òð6?€|QrÉ©…?)ç°QQoÑ?FÁHm¦Ê?y¨ù"ýZ)?–'
$	ù?îi	o˜B?óïèÝq?vѱcÞ÷¬?jmàÖ7¼Æ?¬/9<Šœò?ŠkàÃYƽ?ïÆTD´>w?fCmÍ!í?(VìHŠ?%ÿ°30Tf?|&E^€M?f5›'ÝZØ4FGL J2227.9+0036¿ï©±ŸtÏáÀFÞùü°À'À9®GE8ï5À;Í´ÚgÀ@B89,qx?ÿNlªMF?¶
ï×¾ÃJ?ÀB}þÞlÝ@	†)vò@&ם`Mž?ï–<¢¤@¿Û¥oÛÛ£¿Ù²¬…Y›¨¿ÙÕyäÈl¿çr4/²u3¿Ýí¾Ÿb†]AGNbll3FGL J2227.8+0040PMN J2227+0037?ïa$èHuÙ?ˆé¸)f]'?nº`.Pa?j:ÊèKÉ?Kªëzö?…>0‰@?í'ß#M?´¢.'M?&Œµ\?—ÉB­P‡?³D"Ԅ?°Øá€"¬?î,'õ »?–fPúøȑ?~š¢YÅþ?r¿!›?©cš:»Š?"	EÐ?å•VÎí?¨ñ¤Ág>?œ$P%CÞ?"Fmjø¹Y?Ó䁧?§Žíã##>4FGL J2228.0-4155?¶üÿÿÛìÀL¤ÿiKÀ;Óúú݁PÀ<ö[ªJÁÅ@!ø-ƒpã?ü'/"R	¸?Ð`û£$ð?´ñZuÂNï?êð¾'d@fRðÜ¿ïÝÜ>¯¾?Þ?»Ø?ïʵe§ú…¿çÒ¿?›vi¿Ës˜=£úq¿ÏKi W£ÖAGNbcuRBS 1864?ïÆùÝá-?uº˜J"º2?*?³oˆAû?#ƨO
Ô0?{±sõ&Ð?uy[K0Ð?ï©o1iÙ?ˆ—5Ò|9?=ëžìæ"o?VÂ9ÿÑÓ2?"´Ö®"ˆt?‡Û
!ô?í¿È ì]?"Ü_0ë{?t0"J§Ö?m"š³ù?°Äy#òš?"¨|L ?ïjcÒÉÁ»?…D
E¡?9D£ÂøÔ?>¸›€ü·?'O"8¼á?…5Lr¥4FGL J2228.5+2211¿íMÍÈl¸2À=ÊøzЀ¶À:v×ÁóT÷À<Q¬Ô	1@ë9¸2‹î@A©¸ËŽ?ƪ×Y˜¢¤?Ãõµ¹µÃÇ?ûPÔ´!Û?ü«H%2¿p?ïô›?¥¿Ô6«ÃgÉ=¿ÛRDËáë¿éâd®ÖAÁ¿ä‹*5]¯Þ¿ðAGNbcu87GB 222614.9+215540?í}˜u՚?§Êv(LMT?|†­V(è?yDFg*µ?²JÑ.îÒj?¦ŒN­Bðà?ëØ^Î@™W?µ½âêu÷?•Á¨xw©?½ò÷¾@{?»ÌÃcÝ]?²×%IT¹?ì.nÙµ¿K?ì›¬!p
?˜èëYï7L?ˆ œ7|äÍ?¸RN[Ö7Î?—Û?ÈÚø£?æknÍf?¦-SZŠØÉ?®œ0¶g ?—Lö†ÿà ?Ϋ8œÍߥ?¤9«˜[l4FGL J2228.6-1636?äå–È·qúÀK±#öM¾À:m›¨g'¶À<xÐÜüŹ@¿Î´-™–@?'yꧩ?¾âÊ: bK?™l#"¯¤ô?ܶe§"ê@²¯ï;¿ë¬k˜ÕN|?³'«hÎös¿Û†Iû̔™¿áðk֙տãȓíˆ.7¿ÚÖ Ř%AGNbll3FGL J2228.5-16362MASS J22283018-1636432?ïì´áŒoR?TÇTp u?,k Ö'Â? ké:Rþ?a"lq³L^?S¹Š·:?ïÜç]Ít?xÇ#ÉÏ Y?" FRÿ?-ÀwFª?q=îÏÿùv?xvÓ×ÂH?ï<ÇðÿdÜ?|#¿ÒDþ‡?g`²?Q?b1pl|êG?•zë˜/¡f?xêß	ºc?ï×àç'?XÞ*…ȶD?0²¹ÏÁ«? ª¡Ž!ç?sS!úÑ?XU3—ø4FGL J2229.1+2254¿ïPdô÷8[À=M5e<š»À;€€ÃàÀ<ž£;M@ ôáÊà¹i?ýá©»Þh?Ép£×
=q?¢%¹øߥB?Ø:€›k?ö¢<þ?ïü±a6{½¿ã9 Š¤‰¿è»ÞÓ_Ž¿Ð"L€a9V¿áÙ|"MÀ¿Å\Ùê¦ÒAGNbll3FGL J2229.1+2255NVSS J222913+225511?îû£Pû7l?°—¦ê…?aD©äq?'Øÿ-ºíW?žh­K\"k?®ÉÒbÔ5˜?íÁ]*lÀ?³6-ܸ?v›ɶæ?"ñEqÿÚ?°ˆìïþ»?²êšñßx?훈ÉýQ?"^0©±XO?rIJŸ¨Ô?c†s.ßÎd?±ÿ*o¸ê?"ŒæH(??çü>f9š/?ª7B»Õ?üTÒæ¿?'5k´ž–É?ÍüæÜ:k?«)–jÍA4FGL J2229.2-6911?ÞÖ[8WVËÀE	 :2+À:–(òÀ<~•rÃkû@ÊIÞEp"@_þmXÉ?¼L^}cØí¿©"¯#æÜe?ì!$þ<0ˆ@æ)ë
û\¿á¸Dêë›Å¿ãB;䳿æ§Êêt}€¿å'Paí/ï¿ê÷¢cl·¿ïÿ¦¶tFAGNbcuPKS 2225-694?ï2ž)Áži?™#ãExþk?s'DHÂnk?k'i7ðt?"Ë©µ›—X?—Äd÷MŸ¯?ïEŽ"–¹Ñ?"W‡ú䀕?K—þ˔A?UÕ{
È?–qrí2iw?'ÅÁ9òn(?íù*5vzÍ?"GDÿۅ?ƒòCgÚ§æ?uÜ5=׉a?«pËΡ©C?¢³÷Õ]½?ïEAeus?{ۇÁjÉ)?s3;?‹§?`ïÈ•Ä&?'‹îgª?yåmV˜–4FGL J2229.7-0832?ÐB/*÷
ÊÀIÚÃ.¾YÀ7㸫­˜TÀ;¸<ù…'@6r$àŠ@ÉWòÓÈ?•ŽšPèj?¹^¸`óϊ@þU@ÓfI`I¿ËU+«u+¿äœ.܌¿è]º|h0¿è½¶ÿÛíÒ¿ìÀ©s+pÇ¿ëêM`ÛâêAGNFSRQ3FGL J2229.7-0833PKS 2227-08?ï´ÿÈK³a?vhQ<GÜL?fÑÞ-5hG?c}Söd'?z,˛?qýˆ낞?ï}ç€EI€?'{ÒyA²@?R™cC£êÖ?i–2²0•A?Ž2ó†9"¦?wÂo2Èø?îák•CØ»?çÓ'Y?ŒÈÉܼl3?†²‰1i/ ?•n(i&²‡?†°lњ¸£?ï삾ˆYÍ?T»Žš}?Hw#ÈĞm?CZ.b~:?Z¾ñ
ê¿?Oo0ˆJZ4FGL J2230.9-7815¿î®×"ûÀB="V!uÀ9ü›A9†4À<NB€Æ@$y&5@*t:dÜ?¸LêijÓ? §½sñó?ääýp-º@
›™pÿÇv?Ú¾..½¿ã²xÞ8/¿âhrzpßf¿åã¡$¨Uõ¿àyâš'¿ïÿ¶cÔ»¯AGNbcu3FGL J2230.5-7817PKS 2225-785?ïÍþ…©!?è3!`?FÑÒ´è"?K¿¿Æ<WÊ?v&šÐéÓ?}҆È|â?D–ì?‡@·RJ?3Œi±!Ëê?C°É"T¿?‹ý°Q6Ï?†¥ä!ÚU?ï쨕!ç?ˆJĦ?nñ\¾‡?`®hŒd?˜"J!ÛK]?™»l?ï[}ïsç?vgæ$0á¹?];ê6Â.?J‰b¢?'¼`>?u…Äì|½R4FGL J2231.0-4416?íîÞr;±²ÀL5'Ì÷À9ÓÖxG9zÀ<†óEšN@tu%Çe@8TÛ#§¥?±vp_8Ÿ¯?¨œêB9Lj?ðxë¤(hÕ@,(¡3ìÂ?ªÛk¡
×.¿â}5´Âë¿ç "¦£m¿æðÀ'+ç¿ä$?	ˆ?¿áüâ©­ãÓAGNfsrq3FGL J2230.6-4419PKS 2227-445?ïëò Mä?]°oÈ®y?(A¼°þv?O¸Êy?b‰D=ÇÉ?\ìhéÕ?ïâíTÑ1?u7R'[Ï?Ï×ð^¢?4IcÕ¾?lZ4¯ÁK¨?t"à˜="?ï@%"ó§?{ýâÊ,Û?f(Êí;"¬?R͊»ôuœ?•64#ã«×?yÓ®TÐ(?ïû¯{ޛ?1GËa·S?®+ÎÇ?Ú«ÈZ?>_û†F5¤?0LkæÁêû4FGL J2232.3+6246?âa«'¾¯@G"#ρÀ9¥s¶±•À;M`ÈW@b$uÖÿ@Q*Dw(V?ËE$wX§?ÅÍ£À#@w]š
_?ü…ktm:@?ïÿôa¼2¡¿ÚlUÿø¿è#†b/J¿åha}ÉY{¿ïüG¿e ?ï'[>ê÷ZAGNbcu8C 2230+625?ä½Í°ÅÜ?Äô+È
GÚ?›'nÆýÀ?™.WçT}?ÔËK÷²j?į²mÛê3?ÍÖDÜ eö?ÅKqÅóô?Ãø¦ä©Ž†?Áˆ"˜Á³%?ãŒE­'á?Çrt´@s?ÕemFj¥?°Põ©ã*?¸¨~k7
d?˜tm÷ÚJ3?â89cÖ?°œ¾0ZÉë?˼g¨ž?©Ú³G¸÷©?ÇtÝáuý?°»ÎBÆj?ãKˆÞ_û@?±sà'çÒ4FGL J2232.6+1143¿ÜôBL¬µÀCJ¤ÁëÈ;À5pP‡×ÐÀ:{ô°@¥@ÖÁmH-@–™â"µ.?yW§lý¤?µ^¢¢¬½¹@9–x?'æ@&sg»Ðü¿Ë˸e6»~¿àf·#îÒ¿ä¿ëþ@bF¿äGÊß·¶¿é®‰`‹é¿ì¢úkkˆåAGNFSRQ3FGL J2232.5+1143CTA 102?ìĝ'Œ°#?µGË ›Þ?8'¥Ñ¤?œTÈúI•?µÍù±
q?²Ão²,I§?å™%Bôh"?ØVm¯NÁ_?Ðu¸yèë@?Ö_n0DÍz?±_ô¹Û?¿•4;‹?ꌼ"î¹?±Œ?¢'Ec?¦ý"·3<? ÙÐlç?À
¨'€
?°]8H,ƒ?è'¬!è"î?Ë՜<c!ä?­¨Èã¸nw?¹õ§áÃFÝ?Ç÷?o"ª?ÆøÀɑÊ4FGL J2232.6-2023?î;50l ÀLÓ²VÿÁÀ:ä#åGîÀ<›OÚ2æÝ@ 2ÀD©'V@ÒÁ&¦]?ºz#À8•¿³"F|s)?ù/JUŽ§Î@P@à'¿ÂËr"¬Í~¿è¨nÿ<5»¿ç¤Z¬1¿ÇͼŸ9¿ÜÔWZ¯Îå¿ÛLyÊÇ9AGNbll3FGL J2232.9-2021NVSS J223248-202226?ïÅØJ²Äâ?wˆ©´èÁ?B³âø¤s?4óL—ä…?z½yê>zU?và¸ß"û'?ﯫR°£¾?†¼Ì*¿?3NŠLÈ«Ì?E~½¸†û?ƒz·pË?…ýmJ?îic#ÿä+?‹æR{3•?lÏÐwñ'?Vž‰&Ñ[?§©Âú>#?Šáðªnh`?ï-·Ÿì?'¨·¶V«?VtõŠ"iS?OXciwY?˜Þßã»Ò?'QYõ'4FGL J2232.8+1334¿ì:ðcLMÀB›3ÁÎl	À;{]š
_À<»£IEÄ/@!§â^¯bÚ?ú¯4^¬^?иn¼ W8?¾õCŽu#C?îõ'àh@žwNëö^¿ïþ!¾–©$¿ïEHßlâ?ïÿùëñ¿ÍAÒ2g[Y¿àÔ£éտ̇é­WAGNbllRX J2233.0+1335?ïØ;ÞϦ´?lhS‡?!'tÇYÇ&?.ѐÕ&Y?sU|ññ×û?kâU‹'
?ï2t:¨n?—¡#­Îy]?KÎÍ¥€Ã?`H'ÐN¾?˜Ó¬…a?–¥-H€,*?î
h¨ˆBx?Ç˜
ÚÏÂ?hA¤~¾…?T !5m¾P?­¥[/ø?g›'È?îMûQ'îq?'ž	;D~³?@éj±êÿ?>/‰Ÿ‡?ªÜ¥EBQ%?'‹ýŽaݺ4FGL J2233.9-1229?
!ÂÀKV®Bž
BÀ;"k"ÌÐÿÀ<™êBÿY@=^ú·@É?þyòoÀ?Õ<ÿD™7?ÌÈm×ôÉ?ôré+¨$?ý°|Ҏ'º¿ïᕱ­Œ–?ïöUç¡9¿Û(øýWY-¿Ü!YÁèBI¿ì‡Ø¦õ¢¯¿ïÒ@tdUëAGNbcu3FGL J2233.5-1235PKS 2231-127?ïˆ#õÑÃ?ƒÐE¾ã?`  3Cè?Z$Hæ¶,ž?‰ï5º•/?'JŒ•@ìR?ï6SÕKs?•äwôÇ>?]½Ôñe%?h_kê	¯?—YÍÈ{^?"6ó!Î_ù?íCŒ‰}âœ?™NE®µ²…?–ópO5	?ˆüs­Ö›Ï?°&¿³ýÕ?'h'¬²?íµp¯ŒY?"
tºÁée?…†ÈìØ»o?| ÓW¦¶2?¯GBÌ@Ú?'žpê[e%4FGL J2234.1-2656?ïšK:õ†ÀMî£À9F®×ï?¾À;ãð/¨d8@>|ÔçÎ[?ÿF7õÿÌ?¬¹¤?ԛ?²Râ¥üÿE@4†º™Äb@[ùëñ¿Ö9Tç¸á¿Í6ºý–š¿áÃ^6=¿à÷ÍAìa¿à¿ÓÀí¿åÚI{«AGNbll3FGL J2234.1-2655PMN J2234-2656?ïõ¤•?H¥øÀ·?ÿ*Cfr?˜"ò´[?TgôŸ•
?G׉¿Æû'?ïàx™"ž?w/hÿ#]?"¦ìÕ ?A'õò–-‰?nfl3,Þ?uþþÀúÅä?ïnǓûÝ?"ÅQk[?p®'v‰Öñ?kËÑÒ+?™&†oޝ?²w¿VœŒ?ïïy­{Áh?L/qîη]?	³°Ëj¾>?æF빬´?`ƒÁí4?KÔÚ>¼¤¸4FGL J2235.1-0623¿íô;‹=Ø ÀIʱþë-
À:ßó£Ñ+À<"ÇÝyÃ:@ãܚJC›?ðà"¾ŽE©?Ûy—¹>Ð?ïm8bGõ@æl£—I]@ä(Þñ¿à¥TþŠ	.¿Óiû±¼¦¿ÚÿÔač¿Ú®b¾ç	¿ð?ïÿÿÊPËAGNbcuPMN J2235-0623?ï¡mQŽÿ/?ÍŠì ×?^·çÒ?q[´2¾án?ƒÍÇøƒTq?Žó®@C0'?î_ƪ뵗?¯æ"$5<Í?'UQ£Ã§?›xzÚ@)Ã?¥n@èSàè?¦/g,"Ë"?ë}Y	Bç?¤äÿÖµF?¨Y‰¶Äh?"×âw/'?·èrډý?¡%EC¦?íÆIýTr?¦œQ–ß­Q?Uä'fÀ?SQ1ÔÆ?±v SÑñ?¦'˜uðd4FGL J2235.3+1818?µu¸.À@ìƼèS;À:i"6ÆÀ<h·'"…@ğ+ÔÅ?ÿƒ†Üþ?Ï¡Ñv¹?ЙäB4Wö@RóݲÎ@:äßJ¿Þ®ïÔ;V?ўY<1^¿ãÜÝ¡0fпÔ<_p#¿ìaÈ"n·¿ïÁmž%øAGNbll2MASS J22352860+1816356?ì}G¤|À?²U­ç.ß?'¤ÕéÁ?Œa$MZz?·ªz<fŸŒ?°®†ÿ;r?ïÈÞ!r?šðÈÑëI?`U9ÒÙ~?p!XZ®J?œ|=Áv"?˜âí~…Jö?ëÄŽ'P?¤-֑s!?¥g0ýŒ~?•Ñ½È&ø×?·0GvÿB?›
;¸"u®?îJd¸¾ân?†ÆMgô(?ƒÎù+ˆKå?q°sr=C?¦eö)/Æ9?"3–[§r4FGL J2235.3-4836?Ün;-8ÙÀL
×6&-À97½8SLÀ<YÑ쒛@¬Ê"ùT?@o`àëh?¤Ý,ÁT¹?–ä&¹/ê‡?æãôÑΔM@Ÿá∠οÝR°[Ò䔿âÇZ!‰'¿èý'¬¿å"]àZô¿æ4²G^¿áHrÏCAGNfsrq3FGL J2235.3-4835PKS 2232-488?ïé"?ø´ó?cSc™ÚT:?&"'#'Ê?O}Á?ewåû‡?bÒ ß^?ïÙWUøš˜?³[X¶)?%&âœQÕ?QsäÅYO¹?r¨K̝Ñ@?|ª,µð?ï8ìªT£?À@	~Ó?eÏÝ2"w?Zü›ýÊ?–(‡9ǚö?~:ÚÂ0"ó?ïùvJóÌ:?;¸»ºÉ?&ûPꕛf?ê+ä"ý?Dgÿö)´Ê?7Ô¤ÿ}/4FGL J2235.8-3627?ïñ"G€zÂÀMórq6¤À9}'OH<°À<\²ò03¤@§Íęw‹@Qæ­j1?®Ø\fÍ?³©/¶@ð{xFb»@
C+ò!?ÝC›=]¯¿áÜ®ÙÄ­¿ãOx¶Ë¿ã	U~·–¿æ`ai§d¿ïýüðüAGNbll3FGL J2236.0-3629NVSS J223554-362901?ïã!J—¤Ž?d/5u%	?3Ï)¢T¶‹?,ÅúKLºµ?jdÐ4ڐ?cL§,Ԑd?ï²ø«qÑ?ŠùȑT#?A"Â#á9?bÞÛFo´?')¹9M©?ˆž2a¾¨?ï@ƒ"ðBõ?{7ÙD…ð?kp?q¸ar?dSNnly?"…"À•?wŠòò?ﯕ#ÔN6?iÓW7†Ìþ?eåa"þŠ©?U[`å¹?}B½Kٟ ?dSZ¾ªªÕ4FGL J2236.2-1706?íûµ³çµÀLŸºˆ&ªÀ:'Û ¥&–À<k—€º¥ƒ@øےbm³@›ß>¿Xp?¸2Ó	'¦?¹•b?äض%ö@<ŽP».?ìÎø@n?¿Õe;Ãûm¿ãÝK8)'¿äúm^Ó!¿Û9æ@;Yr¿ç—ͤ?»AGNbll3FGL J2236.0-1706PKS 2233-173?ïœñ/í¾?"š¶ñ	í?h~ wvé?]¥_Ï# ù?œÉòóYP?'·ƒ
ƒ
?ï\ò7.?Œ¾f}¦ÈŽ?AÕ\GqÖ?R«cJS$'?ŠËrpb?‹Ð²ÛDæ?ì¹öÄv?š]<â?Þ©™ƒk?~ºV÷Ü?µøÍÏxãz?–åKï)q?ïúVR"Ò?~Lš°v@?tcp°?d ¤Í?˜[\Y³àî?{–J€¸Œ™4FGL J2236.3+2828¿á¥eeñ‡¨À9¦M;òõVÀ7Éá|‡:À;8œÿ¨@k'HíYµ@*ˆïþ*=?˜N𪢀?ºÄñŒܺ@ Ú£ßm¹A@@Gbj-p¿À¨c¶Þ£å¿àz¡†Íå¿ãwœ¹ßŠ?¿æ#… êÚ¿èqJÝõ¿äy®ý®ìèAGNfsrq3FGL J2236.3+2829B2 2234+28A?ïhÌQÀ7?†Œ³prfÑ?T‰Ÿä¥yt?N8ú­Àò?'å}¡Š?…êç´·Ø[?ïM¸§¦†T?š<¨û"ô?]-^6³À{?ocà»Ì~Ï?"v'Ãù]?™ô[÷?ï,ëfïS?Žc›Äé<«?'¿Ýü&i?Ÿ-U#˜?"1'¤$'?ˆŸÊ>è]|?ŠÄ\e?tj§/Ù?b4¡:
Ñ*?X5''°%ó?'Ž5er´?pÛÑ΅\ø4FGL J2236.4-2309?ɟìAå±(ÀM¥ÈÉ2
™À9á^"ð•)À<drr
c–@l#¸ìÆ@P%çñ?»D?JÑ-?¸ŸŸ˜O?õ2cʪ³@uåµQ¿ãSe¢òð¿âµl]÷,¿êž€‰'\¿èl7`¿]¿ïÿpŽ• ¿ë@ðàþ2 AGNbcu3FGL J2235.6-2319PMN J2236-2309?ïòºÁ›»6?\¾˜å?=QšXN?Fj:uéz'?S62ví?Tš):ñUh?ïºÍ1¯b?†}ý¢¢•©?: Q·?YòVlº?€|~'°®ì?"Y(ˆÚª?ïLä¾»"¬?|lGÌ¢.?k"¢Î§Â?b±ÓKµŠÚ?'òåt5•X?yi#¬È"z?ïÒ»q蕠?bͤ֟ã?Zß©|T©"?N˜êí7xû?oÔ¹Y@‰?\énÏgqï4FGL J2236.5-1433¿çA¢h0|0ÀL›ºÜ	À7™šFgÃ^À;R; g@Úô	Q¸Y@"3ÿ
z?–A…s"?²-í_O¬ø@Ï⾦™\@çv¹iÄ¿ºþÜ>"Ë¿Ý 뽨¿âÔ"Œò¿⹁@‡Y¦¿æ€ƒ}Îaø¿èי¿"9áAGNBLL3FGL J2236.5-1432PKS 2233-148?ï­D¢ÿIû?tí¬yØìñ?>±%yü€?6¹Dø¹¿¥?ƒ¹N]?t}fG®€<?ï½/ûee?'ÆCƒ?7á¼bq
?Oº²Ý!?éæ‡YÆî?›¯|+ h?ïAþÀTåô?‡¹}AkÂø?zpÿ_y?z¿œ¿ÝM?'$"°ci"?'~Lm´?ïñ…ˆ¥-?NwHwKé&?j0?´º?	yŸÝ8ڙ?[ë/±­W?NÞØ7±L4FGL J2236.6+3706?ä,8 /ŠÝÀ2c¥]:ÉÀ;A¹'ÔZ`À<šE'±H@!þ75Ì?´?ü<b¼ºh?ËóÍ–&?˜ÃOܝ`Š?ÏÃYª¹Ò@k,†›»?å!͗¿áìv0í¿âeˆðÔê¿ã<`®kŽ¿Ëßõ½‡¿Â"3£ñaWAGNbllNVSS J223626+370713?ïm'z<"‹?ŽÐÇT?@،ܴh?7z!ø¨Á?'ÆìQ‡Ë^?¼²òNóž?ïL¶hE¿¥?žÔAÐ:©Í?JR\†kÌb?bÌëG'ol?•– ­?ž%l¡Ñš'?í𞝳í?•è-\Ë'o?cà쐢­ð?b†Â	I^?¯¸[·&?•¡úhí…?î¨X´ò	?™ÄÆ~'äÛ?Jš|K7&?EõÚ
.¦Y?®›ƒ"i?™å,X}Â4FGL J2237.0-3921?êF낫§ŸÀMË~dž<À:–VîúÀ<ˆL×I''@léú=|@–Íl.ýD?·üß¶´]?µy™ßd©ù?ûÖÃƓÎ@՜9\-¿â¨+BNC¿â«ï§Ã(¿æ~¸—·¿ãÿL±‰zh¿ð?ïÿÿ>¹úAGNfsrq3FGL J2237.1-3921NVSS J223708-392137?ïôäs;9?Sœ¬wQËh?.°&Q?&Tœ'¸Íþ?Sþ3c‰*Ú?R=x"»R?ïß®«$?wËçgw?%Gf¸òR4?BÍ@ŽU-•?o£Úé]·?vIn)HžÜ?ï9ÒËB¿À?~ñôµÖ(<?pÅ¡®Î"?m(d@2mr?""e¯<Ti?zMœc½Ó‰?ïúu†µNS?8Xy9Óþ?Ê%èÞMC?7Ý×?k?D mªî¡?71Y"14FGL J2239.2-5657?ÛÙÁ†?ÀJã—­À;o†§NŽÀ<ê>Ä`î@cŠ!+ž¿?þ^ã MèÁ?Ù%™A¯ø¬?ÐG¤"Y@Ž?ù–p4Eê?þï~'£2?ï²µ>»§‹?Š8=3<B¿â :<½¿á°ìœuìì¿ïêë I÷p¿îå[n»Ÿ~AGNfsrqPKS 2236-572?ï%ö‰U?'¤ßš–1?kÔ3?U\?r½Û²~š1?—ø¨mr?'4‹×‡¯ù?îȀ·»Æl?œ.ù3?gŠÙÜ ù?qâÇyû/c?¡ÿFæy—3?š?%–Èò?ìD´k¿æ?ŸqM¿G«­?£ç]2§?'?'÷éЃ'?³æ®
.a?"¯·ÏJO?îUVÍ]?ŽŠ´¿­]Î?}¤Y'ídJ?u¨Gq,'ý?¦öž,z'?‹ªáx±4FGL J2239.4+5130¿énì`ª©À¾ºñ6;À:!K,F°À<N0å{@´Î3@*y]¹ïz?Ç!'al¯?Ó]‰Þe¦x@+‰>@+±ÐÈ?å+$;H«j¿Òë!Cœ¿ænÚs~|Þ¿éÑÇ"hà"¿ïÿÅ}M2¹?áEUt¦›AGNbcuLQAC 340+051?Óµ!~¹?¬(Á¡?œ+¢ëK³?"ΐìÍ;V?åD)šÅç?¨Zív9?ÝI_n£U?ͽ†Pwç?l°ö2è´?™J×ï?àØȗ?͂
%ŽsA?ã&J8%sï?±^/VoÉ?½.®æ—Ê'?žÙx?Òg¿Ö%'?¬ût#½Z?ë&ÈɈ¿ô?¢š¸ÜxÖ(?žMý~?†(܅¼C?¿6Vnú¸{? Ô€ý+n4FGL J2240.3-1246?֑)"D ÀL
{é…jÀ;WÓpóˆÀ<Œå—ží–@ åp…ùÿ‹@?ßÁœ"?ÃCeÛQ¿¹µ	a¨'"?ò…Šƒ| ã@ÈæšSRã¿îéºy
2?ïœ&Üã›E¿ãŽñŸêì¿ã¶,ýx¿ßS€Èп¾`ÍöŸAGNbcu1RXS J224014.7-124736?ï5ƒ¸6¦?›2mðÈa?`€©8à?a†N|è?—L›¸äA?šÛº¹Š?ïsvÙ×Þì?÷;ƒƒÝ?I@,á¦{?[u"ÄäW?Ç#`Q?ŽoäfY?í¬êŽt?"âï¬èŽë?x†ÉN˜]?f{ùùqj?±£ʖe?"üÒ4…?í€"í£
?žÀsÄ2Ƽ?r²z¨?z?lŠhèûÛ?²ÓÀèg³ ?Ÿ«·<4FGL J2240.7-4746?ë鍁w'ÄÀL¡R}ÔAÀ;Îj[¾mÀ<Íëýê|
@ð¼~ ïÏ?ÿÌQ—¢H•?ĸ[%À"?"bk¸"b{?Ð2ý›¡²@ÿtHQRƒ?ïjà"'¿ë£BÄ ®¿§ãØ_°J¿ãiÀùYó'¿ÙpÁž›a¿âÇP÷iX‰AGNbcuSUMSS J224042-474733?ïh«¸G?¤E	áÌÊ?Mysú%£ó?FœdV¼Ž1?'ý7Ê?¤4Æö]Â,?路®wÀ?ˆž±/Rp}?8(7*?PA…ká .?†;&<?‡·ch}£?íùO¹µ½§?•ÚíӇb?rDe›«
R?b£ŽDQtô?®"w±.Ãç?C¥WzY;?ïeá¼Ja?wLxŒ	Œ"?N6{?6­?B_Áµr4?'R¥ôº?wD';Müs4FGL J2241.1-4122¿Í
a"ÀÛcÀMä|"µÜÆÀ;úd­(—À=‹Ydö$@"'ÌGÂ?àZ«n®4?ë
¡äÁ¶?ïÿ ^¯¸À?þ¥nij&å?ûmQÇÈÖô?ï¢b€}¾È¿éªÀ2‹¿áÓ¦¥ñ–±¿ÊLœ»·ü†?Á.èävã¿æ)ù˜Ý±÷AGNbcuWISEA J224103.56-412155.5?îþí–;?°ŠìqWœÿ?x³Må(™?tå_'ؾe?¬‰´T‰&?°6>f\\4?îÇ»ö›†?°Ýrb$«?w¢^€$Zç?•±2"qÓ? ôμ9?ª4r¯mù?ì&DD~? ´˜3Æ~?"Uª£áúl?ˆ4R-'?¹¹³4ãu?ŸV!ÅÒÎw?ça–µŒÜ¨?¼Jgè%!?FՙF.óK?[8d"j|?Ñ1gÈC/5?¼Q»DÅì•4FGL J2241.2+4120¿æ`œ ½­ÔÀ.bdä†&öÀ9×Ϗõ«éÀ;ç¼SØÅ)@Bðòç>@n?©c;?¶‹&å#ø¿gï¾d5Pó?²—Ð¸"±@wwZÕ?ëߟ¢È…¿ÌÖÒI¹\ƒ¿å	€¢&Ûâ¿àvé€â"‰¿âS¡2OB¿å2_ê pAGNbll3FGL J2240.9+4121B3 2238+410?ï©Ãð:nˆ?{•'—Wì?UÏöB¼!µ?IÔ¾Þڞg?'Õ)ÙÊ?y¬ìUù‡?ï¡Dpê†H?‡û³X1·W?<è6q0?W"$)?†Îlƒªæ&?†É6J
èÜ?î4ë ¯'?—•¹Ó3?yš¥§÷B-?oE>¬Æ?©"Œ˜öž?•QƒpYƙ?îFŸ>ÖÚ?‰o§P!(ð?wïÙ§±?^ïüݏO?¬½²0ñh?ˆ6wæ¨^4FGL J2241.3+2943¿ç
-žµÀ91jœV|À:ÂðBóš—À<{""i·T@ q/ÓØ.Ö@óøUӍ?·IËù")¿·ó¡!ù$@Ú~<F@üU8k¬K?Õìmçd'È¿ŠðÔqlù¿å×4ó&Ô¿æä>ÙY£
¿Ò×'™¡ý?¿—Éà´5QAGNbcu1RXS J224123.5+294244?îÌN2I¼?¡ÂžL8ß?]KÎdï!&?U[øI"?¢P¾lë.?¡Žü´ºëÍ?ïxcðM¿?›…•s·:?\v
¶QKï?uæ¥Yײ~?›	'Ö'3 ?—þÖru?îN'â]‹¾?""JŽ…Q?oP¹"¿ÎÅ?dÀu­'?©!ÖGûGD?'Pôå7‡?íÄAJO·?›7)³+?j`á¨f>?c–ùCa+?±
ðm ??›X ّü 4FGL J2243.4-2544¿ïÜJ"…]oÀN²]yЦÀ8ó犾4"À;·ÇHÿMS@TXD9ÀÁ?ÿú¨W¢~E?ªñ#
Ì?ÀÝU@w­_I;³@S¥m¼F?ïÿÀà/€ ¿Ù?e*)¿àaâއ	t¿ã+Ñà2_¿çÌéhM¿Ù€/»."¾AGNbll3FGL J2243.4-2541PKS 2240-260?ï@mf¤Ë‹?•÷@{ƒ?aÑô­?dUϗƒöx?•À™
Gø×?"šˆfg,?ìžóci
u?Á°½ä³?¤îêÀ‡†?¹Xݦ¬'›?°'[oWPš?²äm'£O?í|³¸´?£,~?€? Iü"§_Ë?–Ìh ÙÙý?­þ8¡×Dõ?›jrñel?êCúÍ?£%M>†ýœ?˜Õ xÝì?ƒ[Ùÿ???ĨL°5?¢Z5ô¨¡¶4FGL J2243.5-3931?£Aœù«;ÀN`:!cýÖÀ:‹ÆÞÀ< 7Ǫf@½ëf?úí@w❪?ÃQsûz_B?¼BÎÜãÆ?ö¯Äcq¿`@E3²_
W?Ŕ€ãÀ.¿äbžÍ¶¿å$¨ Eæ¿æy¦µ¿è%Áۂ¿ïýݱ žÜAGNbcu3FGL J2243.2-3933NVSS J224326-393353?ï/QçCG¨?"uߍÛ(?\Cfÿ/¤?W`̟¤1‹?˜QŒ§¦?'Ž8"2I?y;!?J¨Ðã—Z?Im鎡Ÿ?[ӆܾÜq?½ÝÑ(MÕ?Žúx™óŽU?î¾V<"†?‹öê«û?q¬FžLD?`7~&'Ï?¡åjt¼?ˆ–	~²â\?ïWuü5›í?uû¹ˆq{?joý/
¾?SÙzf/ö?'Ã@Ók?Q?tÕÐ-÷O!4FGL J2243.7-1231¿æX«ÎâÀL_9&A³À:pûëžÀ<7ªËñ@žhJí6@‹SB3'?³ª$>®ç¿±±ß‹–K±?ý÷½#â]@~矕¿âu	—Xw¿éxHÞ½¿âD­Cš‰"¿ãS{ýýFg¿Ñ)O¤Øçã¿à³ã'/ßAGNbll3FGL J2243.6-1230RBS 1888?ìžeØI4È?³ø¡df?€֙1`?y\¾Ÿ.?¹Öj9'?³‹òï¼S?ï#—MöÄ ?›/âZ#mó?Z0§ÏÅÉ?k³;œ"?™êÄ+N?™a—Ž†9‰?ì"¢¡GEj?¡Y!Ž?Œi»ªžíÎ?~ZrºÞ?»]³€qöõ?Ÿ"z7_h?ì©à®ìô£?ž0ë^²ÇŒ?r×?aœg­?gfˆW–Ù?¹ƒ†'~"l?ž_–—ú4FGL J2243.8-2510¿Ñ訁ÔÀN¯'Àa"À:~-o}À<
qäHêU@M¾—@iÒaaCè?ؤó…?ïÿÕm…>™?üªáÀyØ@`œ¤ç¿Ôúҙ•gÜ¿â ç×Nl¿è±¸¿y¨
¿í•
È?Ÿ¿»{šâD¿ïûX0B½ëAGNbcuPMN J2243-2505?í¥*C.?¶"¿©u³?¸Á4?‡}MzYÂ?°Û,—ô[?´àì+Ç ™?î†/SÔÀº?°¤Äð0²?ˆŒì+Šƒ?Ÿš¨†«?¡yÏ·ÔÂ?¥¼Ãž?ê	sÈS?«§zÎpÝ?¨§±  Þ?—C0ã½?Á±ÍËܧ*?¦…œ–Ê.=?í'{F+ý?¥¦L¦
],?`R«§Ó©¾?`QA¸8V?³ir Ê?¥{K$À4FGL J2243.9+2021?ÇêK£"ëÀ@®÷S½À7ìõì€Ç;À;5ìlø@L·
Gç?ûrÀç¼<\?þÞmÅ<?µ®_4ª@qØ¥H#…@.G«æ"^?ËѺÀ/Û¿¹^f'±¿ÙrԞReþ¿ÛØz™9¿Ý¥SŒ¿âpY.oAGNbll3FGL J2243.9+2021RGB J2243+203?ïؔ›ÓRF?x^hÃZ°h?>3¯!wÊ0?<ûfßÑ?qÒw$?`Ÿ?w[éâ'ã?ï]Q±K?''Ìž³?UyŒ?h›Áï·,û?"e±y?é=s~?îv¶ƒ'éƒ?—B!e[?¬Yõ›?ŠyÖڎÒ?¡4¬±Té?',ƒ"]¡?î
匾?—Ë´Óƒ¤?fxãðb=^?VÀœÕ\ô"?­"h-úA?—§ðJŠgÚ4FGL J2244.2+4057¿Ü1XÀ/šw@Ý@À7zw⏬±À;3R­Kþ@¿AùŸ"@4ìÁ^ځ?"œ˜ëZ?¸³7¥]È@$©?)
»@ »Çö|?¨+Ø ¿Ýh܂¢\6¿áóìáÀ#ò¿á0%⒱ɿæÉñ…é¹m¿èÏ|_LØAGNfsrq3FGL J2244.1+4057TXS 2241+406?ïªW}æM?uÜèCü¹ø?OI^w/2ò?K~QÐ?ƒuŠØyÑ?t§žŠ«tŠ?ï¡,Š,Æ­?›|"£¯Ä?U}fþÐ[±?wæ~ý6‡ü?…0"ôI?šcÓò+ùÒ?î
z¾½éU?œ6ò(=ùÑ?œ¯Wÿ&ïe?'Ã÷)w—×?¡¨òý?"_&à…?ïÐFÍ¿š1?pb?Ïb&Ÿ?5þ÷O¾V?5º½ð
è?v'¹0½ê³?pðñÇîÈ4FGL J2244.6+2502¿Ì€ZÅë©~À=‹T~–À:ÆcQÞïåÀ<"PP@líañ3?üðiϘY?ÑÖï»dD£?ÒòõÀáÜÿ?ÿõ²ÉìH?ùÿ¥è¿å÷É?¤…±¿ÑÑðã'pÞ¿ÞçIeN¹L¿Ø£¹bâ£N¿äáâ¾P³!¿ïÿýF\IAGNbll3FGL J2244.6+2503NVSS J224436+250345?ïtÇp†ïs?ƒqw]4]?VÉüS½c?Pž5ÔM¶?ôäSàë?'¾c¬É<{?í¬]ì_?±:6'쳊?€_gíãWò?‰7º†™ï´?±ö°ãr	?¯óubç(]?ìÚíǗå‡?›$ã?×l?•ík÷Ù!A?‡»…æ¢ê™?³­6ÅJ‹j?•§~°CM?ë$IJE¯ÿ?œKVŸB?Š+~Ôf?{Âr4´?Á]•g%åx?š5[A%D4FGL J2244.9-0007?ïN=_ÜßjÀH­Üa•FNÀ:ìj`Æê5À<CãÎq»@VU7«@pÜ¢b–?Éç¨ìMñ?€}:	Þr‰?³¤ÁÀÕ?ÿÞ½:2¬?ï*2‰}ÿæ֙ŸxÖ«¿â^éÐÒk¿äjÜs­¿åcŽz¦^¿ïù?A3|AGNbllNVSS J224448-000616?ïŠÜÈîÁ`?ƒ/&CÌâ­?P{ûCas?F"ÿ˜. "?‹9NbG;Ñ?'mÅ%õ?﵈E?–6ÖHpò?XLTÇQ?b5â"'—o?›y7àvÚæ?•D"‡?ív­ê3§?"#¦ç"O
?'+Ýnv3?nPG1L?²
&àÀ"þ?'›ñ{™*¤?ì¡Қ@?›þ¿ÓÌ?{«mü'?l›7»0Ë?½È=!©Dô?›'|"+´Ö4FGL J2245.5-1734?ëˆå3ö҅ÀMºõýG¾ÛÀ;Œ8ap]`À<Ô/[7^;@!´oˆÎñ?óÊíêSÆQ?ߙ«¢°™?ä‰ößÅÎ@¦-['Ý•@¸"Æ©r¿ïÿSg†!?ïô…¾Eu€¿çÃÉîËû?ÈíPÐÒëË¿ÏÄãIeú†¿ïöºÂM¬AGNbcuNVSS J224531-173357?ï³aiýs?€hý#9¶?g&®kéÏ?cß[bëb?z»óóC?|ÅÇì¡ç?ïuíTL—Ú?•%i·Ò?Tùâ<Áš»?p&©ŽGK?ån¥AÖm?"L¼É9rù?í2óîôP?—(h}Fä?¦õÐÁv^?'˜?Q¡?²>©´Wÿé?" ´LÊÖ?îkv2/Õ"?"ÖJ²í¶?\™5g­¯¼?]ëj}'¥Ì?¨cÓ1Å@u?""†Y»èÔ4FGL J2245.9+1544¿áFùF°òÀBµ‡aˆ±À9ȺÅ­À<£Ä•Æ¦@ 8`Á¥?þ^ŠÏÒ;?ºÎ¬ l?³[;ùç?ôõ]ʶr@
ÌÕHq]æ?îZÌiÐ~2¿çsø :G¥¿Øýç!¿Ü/›¤
᰿ᆚï/:¿Þ!ƒkáAGNbll1FGL J2246.3+154987GB 224338.7+152914?ïÛIéY#ë?d¨C|IAo?3E»­,:m?%ߘc¯£?q&¯˜›Fj?cýVD¹@»?ïvù"âÌ>?‹ŒR‹Õ¬?@ªsX+?Uš>e!?›yêª
F?Š£›÷fg²?<q­?·_
s?giGh1Öd?_0J‰1Ò?››Ck"?€mŠjž?î)ÖÚ:Ž¥?‰‹F{£ˆ?kƒW2Bâ?T§1¾S¹?«°š&ãñ?‰)%ñÿg4FGL J2246.7-5207¿ÔPW=K†ÀKê¶â—À:ï/éÁÐÀ<E³Æl@!­#>ô\‰?úƍ«?Å<)¦íj&?³]&¡ª_:?ïÊi²KA@˜»ûÄ1¿ïÿÒ†ëA?ïmMá4c?é°Sº'7¦¿ÀãÛ\1¯%¿âñÝ}t¿¡^ÿÝp^AGNbcu3FGL J2246.7-5205RBS 1895?ïè/¬v)õ?bê8Ûù?#I¢ÂàV4?)stJÖT?f›¹]¨º?b†ëÈК?ïÃnC 
?ć4t
Pn?3‡qPÊg?MæÛÆ]?}¥øåé.?'ñ–¨ê'?îbN°Ž¦`?'Ž R¼Ñ¼?aåô3à½??Pcö™'p ?¨¼µ³×ŽB?'wáO¯º÷?ï‰7ÿš@?xքtæÄu?D{ìÁüYä??k™Û-Q?Œj|sùªl?x­ß—Ljš4FGL J2247.4-0001?á‹9ÌvÝúÀHÞí¢/jQÀ9ÍÊ¢P!À<õ¦	ê@aóA€¨Ý?ÿÖxG9zu?¼¬†hÍ?±©`­Ç?ô=Òä>š@Wëî%7¿êÿ‹ /}¿µ~#qt6‰¿ä‰!S6ß¿Öký¼ug¿ãË=€"¿åv˜B"ÐAGNbll3FGL J2247.2-0004PKS 2244-002?ïQÀúvDú?‹I
Ô#+?X±I
Ñ?PäZôfÂ?"<Ì 'Ï?Š ¿;Š¨?ɤ{¥?‹ßÈèá?EãW²Åö?T÷Ö?ŒÆ_aeê,?Š«£p>¦^?íµ\
0¢ç?˜ÿrG«?äèõÈ:v?qZo©r0‰?°VÑe$?–y½)öËv?î'´ÀLQ?†Öü'ö•??rËMÃÞ?` úV@±?¤–‰'‹?…³…'c@4FGL J2247.5-3700¿Óà6ÆÀO쿱[WÀ;q?ÊjåÀ<É(˜¥}Ó@+LOŽÞ€@›m´Zæ?Ö>‡$L?¼oU£J?àhÄÓTÑ?ü["ìÝ¿äCt^v­Ü¿ê•êMT¿ã1¾kàú¿á
ÀþŠÓ¿ïÿßHÐSj?ïbŒ•AGNfsrqPKS 2244-37?ï›ÔåHύ?…UÉ.¡Þ?C€Á í?=¢^V½?‡Òı²ý?…(d³8Ï?ïCŠtû?˜ö]ԉÇ?\áa¶w?q~€× Ï?•Ï¸•ùU?–™ËQX'?íò•qÞ?'ƒ6BaÉÜ?…Î^¾³?x—Íl
'¾?«•ûñ@"+?Ž¡Þ!đ?îþß:™xÁ?ˆ$Üe(¦×?WŽLª¯'?Q¬›ø+Ui?ž²¿È<Ò?‡³ÌÂπ4FGL J2247.8+4413?ïb…-fæÀ*'||R`öÀ9ÄÁA® À<iÍ#3â@!-þËøf"?üb»frû ?³,qMB?Œ#nUY_?ڜb6Uýc@hùÔî¿ìäo¶q@µ?ï<›'Á^¿Þ':_w^Ü¿ßîHÝêVv¿Ízƒ~Ы¿ÙlƒKy{AGNbll3FGL J2247.8+4413RGB J2247+442?ïÃ
Éq?wX~¢³?E}'.|c­?EFËô$û?{ÉÄÕwç	?u´g«:×?ï²\j£;?‡Ð<A[£x?0tuV°€?@Ô×y}a…?'åAÏ!±h?‡s¢ÄîÁÝ?ì»ó†']?ŸØß?g?'Äè'N?uõàÿ¶Ã<?·Çƹ*4+?²Ž:r?á\y?‹÷:žÍ¬'?rðÁæ>¨¾?bÞt0pÅ?¤V‰­o#h?‹Ê·ëfb4FGL J2248.7-3235?ÔP…²¹	ÀOyI@»±òÀ9í|7‰À<iÆú$ô¬@htbÑ@⩓àß?µŽ]ü4™?£bÓd÷?êBlA@\gç'l¿Ð㔤è,O¿ç$`ãð€¿é†Œa!Øî¿èœl^Íì¿ïÿÿ&¦³?ïï?ôÕ÷AGNfsrq3FGL J2248.6-3235PKS 2245-328?ïíF‰ÑÞL?•ØŠÁÀ0¬?@Oo÷ ?i>pãËL1?]K,¤GÙþ?'³¤Ðj1?ïÇ=Ejú?"ÄŽl –?2ԌRÑ?QGÇ:'Ä?{X´…Vj?ƒšz¼Æ
¸?ïP·Ô Š?x
¯BdáA?i'€)ٞ?[úáIm3?'¶üõf³½?uSñ³ä2?ïï²VXï?NFTcV«?:¯ð¢'J?1ˆÃÄpÉ·?YïøB?Jù¤¿Íh4FGL J2248.9+2106?î£ëâ32ÕÀ@±Å3À:P.ŽˆÄ_À<[6@KAqåK@·ÛnP?³?ÂT¶ø°?´÷îc c?ñhãï(Ah@V0´RØ?ïS³çc¿ßifËæó¿¿ãÊ
æ
³¿à5ŸI[ê¿è¸ê—¸ï¿ïýc¾yåAGNfsrqPKS 2246+208?ïë¨%ÞV?j?N/êQ?:$ÕÁÐÓ?Pi9WgÃ?aYiná?c/(
ÜÀ®?ï¤rùgú?…¥‰æ¸»?4*çnçÝ)?GÀŸYÝ3?†AêjǶ?"¿*T\Îf?ï/=RØz?~Y_/
3'?gC´\ ü?Sh¥ÆOÕ?—/ß3rüÐ?|a.{¢4?ïzæÓ{+ë?pdGðn‹?c"SK?M7–á'je?ŒfLpò'?nXyí)4FGL J2249.4-1300¿ïI²¦4ÀMužèóÀ9<äw
}—À:ô؄ô@ OÏë1@ðúÄV܆?¼^z‰³ób¿¡UWv'Ù?ꋾßK@@½àJÙ?íÊt}€^_¿íz	ç	Žõ¿ÅÄyÇÑ¿é4mÙw¿åCå~*¨¿±ó¸žík~AGNbllRBS 1899?î·µp?´6äiª8?Xµžþ?`!3û6?£Éì{€ù¬?³õ«Õç?ïÅž-¨?†o¤#Š?2‹UVÏ‹?KAØÌÏå?|L{"¿L?…¨™ò€ñ»?åmK/Ö¥?³gÏ4µtß?
ÝÀ"¼Ü?'1•'d¿?Ôw—ç?²å9¬&ì…?é|…ñØY"?´·÷€çË?*˜ûn»Úœ?'żÃ0?ÊAùÂê÷?´µáÙnQd4FGL J2249.7-5944?è~•CÀI§Ž\NµpÀ:ãÝéTÃÀ<µ&o<Ï@"W'
3D@M++ý´Ì?ƆîFD2	¿Ã~'Î?Çåóö@áÐj?¿ïñüÂ2êä?îAw^o¿ãP¸7åŝ~*¨J¿Äs6X¡U¿ïÿG©ýdAGNbcu3FGL J2249.3-5943SUMSS J224938-594421?ïèH gâ?^9æ¼`á?5y€7"¥?1ti"ø?eO‡X§‰í?\mS"aº?ïÊà'#8?}¡pð"ë'?¤AU<ý?2u¦b·Yë?z-é ç?} ¼—k?îžßéù?\ÛÍǕ?xlîè«H?e¤"6?«¡x4ë÷a?Ž¨pH¼"?ïÇ:}Pµ?fítûÆ?C@'Ê?<Ås³@ž?zš¯Œ˜?eÇɼÉÐô4FGL J2249.9+0452?íekb‹ÀGJiߗª¬À;;m"XÀ<‰U>öµÔ@ÔBŒíd@£ÿYçÓ?ÁÉÓގ쿦ÆcÉuw?ãkD´e@¿o`
+Ó?ïÿQº÷k¿àšPCrŠ¿ãkâ§)¥¿è»F'‹ˆ¿àñÈ.Ø[¿††="«»RAGNbcuWISEA J225007.35+045617.3?ï½Ûf7±?wÚ¼Ê2ÿ…?@¾÷~a?F={³Æÿ>?~úŒ…ƒ×î?wv ufç?ïr·Jpé?‹Ú¢v"¦?BXXCØ¥?Q×õFs?'+ÆT™,)?Šèd@¯ø¬?î/úÒ'î?Š¯õyÃü?u1¡1aú?f.܇?ª\ì©hó?Žp0ôexø?ï#g³ ò?~z*a`™?R¢!qÈ?G[
i¶?šhýA™Ê«?~I~"íxt4FGL J2250.0-1250¿ï~Dž)ÀM:'£SÀ7`@ÒX'	À:oîÑ"2@ÎmÚÎî@Ìy1D?šw'ç+{a?Á+±I8®@*ç'Jð¿@!¥r6ð¿Å±Œ)™q¿Ò|	°ÛU¿åÁ£¾¶‰"¿äœÂä¾®¿ç€q¿àÖ¿ïÿôA…ÜMAGNbcuPKS 2247-131?îæpÑà3)?Ÿ3cEWsÅ?ýöÃ[`?"èi…GÜS?›2h<Ä:?›'j\jX?î9
0ÒCP?½h&±Ývõ?'f²I*j	?³Á~wݼ?£;ÓÎF•ý?°ƒå ëzò?åWª	FQ"?±Öãó«?·ídáºÅú?£0ó:4­©?Ϊ¥j	X|?°(¤V¹š?çúSÄè|^?Â$_›ñ˜q?|¨A­Üu?'jœä,?Ï63ªPŸ¥?ÁñèÅRè4FGL J2250.0+3825¿äÂ|s¼À2Ô8ÑØ¥À9uTáä·À;ð/Þí@!dèŒñÀ?ûi¥ë·sŸ?®ôMS?'¡Ö\¡Q?ä?O™›G@
}ÙªUÔs¿ìô±d "?ǔ$9Æ_¿Ûguû.ßç¿Ó5dæ´¿âÒÐ¦¿´¸¨ÓsZAGNbll3FGL J2250.1+3825B3 2247+381?ïéPoš?^¥o ú¤?#‹¾œíÑ¢?ĔŸx&?evÄüÁŠe?] # ßH?ïÀ¢%´†o?'†â>@êx?2¾E'¯a?Qåô¹9Ï?~ƒ͑ҕ?	î*/?§ËÿŒ?î'h:ê?hÍêÉý ?WÍ׀YÄ?£xã3gz?fT†Î?î¯çó·Ï.?‡F"ïg
?b
4¹©?OÈÁ_l>?£à°A91?†nÐK¹Qp4FGL J2250.4-4206¿Ôð] šÀN–HƒýP"À:"ë=ÑçÀ<æšÔ,=@ñ¾1""@¨Ú!I%ä?³ö¢3F(ƒ?qJB¤Œ´?À"z~K_z@"`d\?îE ˆ¡#Ò¿ã
AQ®ô¿ãL¦ló"¿à‹,žÄ{Å¿ãb¼ÃjM|¿Óð
H´ÐAGNbll3FGL J2250.3-4206PMN J2250-4206?ï݃dœ?cU÷®]¬}?4¥ÂÙçÐR?#ìŽ*nIª?oè+@&ðæ?bžÐ(dÓ?ïÒóÑkïy?yÑú
Ä??"R|h/Çø?:üî`9{?uóƒfÆÅY?y*ôVæE?ïD×9Šz4?w¾ü"!§Â?có>nÝÔ?LÃ@Òò?•úfâݤ?v¡øxJø?ïÊÄÆ Â?a"ç?Dýßb?1q)
iâ?{ªyüýã"?`âàøÇË4FGL J2250.4+1748? ?²©ÕÀB*ù‡?úÂÀ9ÿI¯vz±À;ü3Â¥@pªEä;@HPïܜ?¶×(˜¿ˆ"¿Ã'~Ó?ÅBÔ{lÝÏ@P",P¿ç%=Ì4¿ëË·XÇAs¿â.LC¥q>¿êaÞËÒÒ¿â£Ó¯?¿ïó¬ÐDÑAGNbll3FGL J2250.3+174787GB 224805.0+173330?íÈ\è÷Uï?²®ÿ‹ï"?S䊮3õ.?RðÛ±NI?±m†Œ€»?²—ñ"çK?ï
8ÃÑ«? ß·PŠã?TKâkò?o¿Åjgƒ?ž§¢Ç£Î? O
»r'?é<m¨!¹?°Þ¤¶+_Å?•ås"€*±?†^Ö±O~Ý?ÈQasÅ?®äurÕX?ì@€? ¿—ˆºª'?d<O厄?W9ãͬ?½^‡3q? º›auw4FGL J2250.7-2806?È#ÇXLOíÀO¨×ƒßóñÀ8{cRµ¯zÀ;™kŸ‹K@#ëÀ š@cTÁ"tŸ?¤õç"c'0?¸abEšh÷@ô‹"'Å@­ñâÝûŒ¾>êw¿ÓÜ#…}ƒ¿â¨½¯"˜¿âo–[ ¸¿ç+úŸ˜â¿ç+Kb©îQAGNbll3FGL J2250.7-2806PMN J2250-2806?ﴚpö£o?u<×J‰C:?=êàÚ:F?8Bù¤¨Î?ê»…R"?t·¨BÅÍÎ?ï×91AR,?yÂõtôÅA?*WÓÝâ"?AaÑ£ý-ˆ?s¨ÀgÙk?xñžÃ~Ï?îr.Tu<?—)'¯ ?†êÊé%1›?"r2ê.	?£"h_´?'ÇÇËäc?ïë§*Ý؏?Rfî¥·‡?·óýϊ:?
]h=VJÀ?c£'8ôó?Rח(=4FGL J2251.2+5550?ï'ñžW2À	MÔº.À:·¶'Τ=À<ž¡@W@´n œ˜'?ø­ä	)tn?Ք#c‡?â5ð²…"ê@z&3pp@"u€4ì?ï·²­fÖ?ïû"€«1¿ã¢à՘Mi¿Ô×DÈ¿éeã>~?÷¿ïÿ
Çhß½AGNbcu87GB 224837.7+553415?îà×`ôt? YÐÅ{š:?}çóp $À?â£JŒé?œkit½?šÊšDr%?äçû'‰?Ï:[…^ô‹?sˆÓºCy"?ˆÈ°P%˜¾?Õáåï?μˆõƒ~?èÃN±I?­ß&é7ï¾?¥·!kýF?'¯m¾86Š?ȋ.<෉?©ñÜĄ?ìX]}I/²?£)\úÊ6?…Žÿ"^Ð~?~6'8Sٔ?º‹4%*¨b?¢µÅÙIt4FGL J2251.5-4928?Êõ6SÀLù¸Që…À9ÂXr‡ÜÙÀ<;€kË*5@ ÛçœÜÅ?û½.äïÙA?´$í ,ì?º—ën£w@QJZ—%K@•#"™Þ?ïØÜx5?ÓÇ3{¨ø¿ÜÌÜÝ;/¿Ñà¤.Èë¿ß
0eMŒ¦¿äâO §)ûAGNbll3FGL J2251.5-4928SUMSS J225128-492912?ïôsGÓæ?TG'4…½~?&Ø,Âf$Ë?#ÐÑZ!a?T>jÁ•rc?RypX'š?ïÕìÙ,RŸ?{2ám?#pɔU¼T?@6Ê{S?tn
4ä?yýÚӋS¡?ïØ(NÕ$?€
±¥ÃA?j9à;½?`uÐ0+¬û?™½¾ò]ã·?|ԄÓÁ®à?ï·G7ô3?gªjíC?DÑSDڛ?7C8
ïä?€íýÁ%»?füÄËåK¡4FGL J2251.7-3208¿âÏSÿuZÀOͳÐ|"¶À;6ªw7oÀ<­[.ú¿N@!V\îm†k?üy0ˆ^ó?ÆÔÏ»¼Ë?g"õƒá\¸?ŠÎ¥rž`±@Sõ.jÌ}?ïQ8×·âZ¿ë©Åá¡A¿Ôìò»ÈC¿àUçÈѕ‰¿æ¶b!Z?àU¹pޏAGNbcu1RXS J225146.9-320614?窱dû?R§³ÇÇ?5ñ.ŠÜPS?0˜¨½-3T?"δ`Þ¹?~'û¼Ö½??ïfZ0n-?•eS}IGÉ?P–¨ªÒ´w?aÔs³hiæ?'+Or¥?"Ëð\ã?íðêw¢©€?'h-ƒˆ£?m7{¹ƒ0?_û˜oÜÚ&?¯çþÏä?Üeï«?í)Q[?žçόA©?]¶Ýjæ?SÙ?}áq`?¶>™³tÒ?ŸÍ»Ä4FGL J2252.0+4031?ä'ó°nüÀ0ã"[tšÝÀ9>Ëò²9¤À<	z‡…›@À'Ÿ:'@Ñ"2w?¯¨Ž¡ebR?¤9¯¤A?ôü…×Dö@	\'»Ô¬ë?ÒÞ&[´[½¿ÓSˆþ–É[¿á–¥ÞÌS«¿Ü|—UG¿â§ýª»*
¿â¡·ªü˜lAGNbll3FGL J2251.9+4031MG4 J225201+4030?ïÏðÁî6«?k9÷'âÇ?B½9{{–®?5JhCöݚ?u¯÷Ùu8T?iÀ"'Ÿ ù?ï·Û…Nî	?ƒh†Aç?B§†SG?Zæ›ÀPß?€Þ¦Gû?Ïyße?ï!7Zr™?~#sÓoë??hÛ²G²O?WUKkql?˜ÁâË»i5?{hÊ`ƒj´?ï¦B†Ç"?£z¼uÿ?z`[?bÆ?nR2ù?˜ãr© u}?{mûúr4FGL J2252.6+1245¿˜Ic'M¦ÀDf¸w«À;<Ÿ1‰À<œ׊•ñ@ lià™]?þúEዠ³?Ê£âëE?½g³¶Ñ?ò"ßq?@@Î*oë¿ïÿýFKê?ïû×ómK?äÜ7£~ö¿çOHÿ΂¿â•Oçžà?µüé=ÝÜAGNbll2MASS J22523220+1245109?ï¯ÒTÐFý?|Ó©Ÿ™ë?@~wòžÇs?8¯­?ƒƒLÄTˆ?|nbFA±?ï5·1¯Gô?"cÊ 7œç?QsCÔöì»?cô¡"¢.?˜1åŒÇ'¨?"( 	¢¨5?îc¿q?ŽëÙýÎã…?wvÓÂBÏÂ?i>C;%
?«Ê閷â?Œœ…£Œmh?îs‰§%"V? Ž"uÞ´?jYCua
ò?i´>ŠÊ?§!ÑVWɹ?x¡¢ARÍ4FGL J2253.2-1232¿º•ø5—w½ÀM]Ñ_ÄÖÀ9ß=ÍÀè"À;À®J*Æ@*ߊ¿¥@ÚøßzN?Ô€"ØA?á©é"mé@›ç¢;(Ë@à{/Ì ¿á×xø9b¿æ=¸È3
¿å¢Z¾ž
¿ìÿ atd+¿ãHY€NïÒ¿ÐFPܼYAGNbcu3FGL J2253.1-1237TXS 2250-127?ì;㦁Ï?·ú(ßï^e?zðÏ­
ͨ?wêTb?¼x#çûD­?·œåIÃ<?î!^ÑTn?¯ú¢vÑ?ƒõ­»@ßì?R"‹ÁòÂ?¢~¤#?¥À'b€i)?çـ0CÛ¦?«¯^1ÃÜW?¬é§—¿si?–†oÚ7?É_•Y´?¨ÄðK=C?ìöëpn6?žØN×_"Ÿ?l¯ÃÕT#n?`u$0ÜÔ?·c&]ãªa?žF'J_qÈ4FGL J2253.3+3233¿°3;£ÿüÀ8	"‰a=À;-Ëë%À<fÙþ
·y@ 4ÓÇ=@o³·RE?ƒìÁ´À¼¿€Ã@ö¯
8?¹!˜¿/@g‡ÒœÅs?ïù]¹ïzw¿ßmµ»
\µ¿à²ž­›¯¿èòÂ?U*¿àq¹KÈ˿ے¤²ÒOÄAGNbcuCRATES J225312+323615?îkŒÄÌæ?£vJEy?Ya¶ð*ƒ?\çm²*7!?¨{|2Pb?¢®õbh³?ï6º¢æ
È?'ÝøúÍ6?RMÏê:4?a{åu–U?˜Ԛ£É?'%r—¢ø?ímV LiÂ?"ŠÑÐëǸ?·–lÎÖ?p½çO"?²^\-¯?"ùê¸?îTÕøg?‡úã'é&O?bl¢?ŠéÅ?T7§ÍÆx…?©‹Ö[Ç*ö?ˆ0=×"4FGL J2253.7+1405¿ïZ­åDØÀCîWûi˜JÀ:Îb«ÆÂÈÀ<v²¹%P@ ¥‡4è&?þLhĸ*?ÇläDb°y?À|êŒP[?õºÂùå3Ì@—dÌÞ?'?îϾB'¿íè¡^ßßN¿¸\2ZñQ¿âHMv«X¿Ý&-;L‡B¿ÙvÞ¸1µAGNbll3FGL J2254.0+1403NVSS J225354+140439?ï#/fŸ'³?"i ˆ6ß?EŸ?§l¬?>W]õ?šíJnS?")iÿƒ?îç|¥Í¡U?Ÿ¹LŸ?ZCëÀÍ6À?j|v~7? ¶E€ú?lÇÞ-Ü¡?íäƒçÊ0?—+ÿ'àÁ?e
œxW§h?Tê§ð6?°3‹ãþñF?–¢û_Oh?ìÉ{oŒ"ó?›úI݉©?dèÕ,?é?YTqeÖ¬?¹ÝÚ7Îm?›õ?à!C"4FGL J2253.9+1609¿Ñeht³†*ÀC©~+VÀ4ºaŸWH¼À:›²xŽ@ˇįó@K̼ܔÁ?|gÈ_V‡?¹¬‹cË×Y@C‡~|â@%ᖏùÞ¿Ìú'WÛß¿â3ÂÚۃI¿æÎÇxÏõ¿æÊֈ7q†¿ëa#0†°‰¿ìVB+ÐAGNFSRQ3FGL J2254.0+16083C 454.3?áÒlt`I?ÉU^§bÑ?°}¸Ô??·zrlE͌?ØTáé
_?Èù',†D?Öpš¢Rʳ?ÚӾШõ«?âØ؉ç:z?ÛºlY¨j\?®í¢NöÌ?¾QOãdº?ã
ۍS¦?º"17¸£?Âs7á'¬?±–ïl‰¤D?Ъ¬õM'²?»Ê}°!?Œ:±EÈu\?£½.±uùº?ß9i²Ï\?ÒYã
/2s?ßå'ìø?Ò-"	²Z4FGL J2254.2+4305?èJ€ß/ó/À-'L¾´À:‹"XÖÀ<Áh¼P@ª>0'D@^e'
?»öùŠp¿p7}¡"°?­xŽÃ8	Ã?â%ébs¿áò_-¿åcŽDÑÁ(¿éÿ½Ñb^¿âíŒM€¼¿ïûS]u&?ï¸d*LåAGNbcu3FGL J2254.6+4253B3 2251+428?ïÅ£Ì(] ?*ê?{?p^æÙrÄ÷?œT—à²îç?ižf$¼Ô	?oŸ¡ÏpS¬?ëÔºªÖB8?Âñ¦@˜¬A?¦×IÝݕ,?¹
àMa«š?µî…º_#§?¸Áó⸈\?ë
ƒ¥ùe?£«"n ÀH?¤a©p|0š?" iݨŸÿ?½{ùd"?ž¢êÕ¡?骫ºËËG?±Rçtݦ?³dÔ×ú9?¦¿O'²Í%?¿EÍQ§"?¨HgÃÛ<Ð4FGL J2254.8-2725?í²¦5^[«ÀP	ÿÖ"îÀ:D¶4‹À<,ü<& ü@ ×0;Üúí?ÿò‹ÿH?ÀœÒ^18²?:燎)N?ÐɒZ¶@·{ý+?éý+4¾y¿çª|?ì¿à»²}ì¿ÜP'¤_›F¿â"?_'`¿ÅÑûÆ_uAGNbllNVSS J225453-272509?ïîem´Ö?ZC¨ƒ4¼<?'"u©žçÁ?~xÿ5‹o?`!Zð" ?YK[Ú9?ïÏ
œˆ?{ê°-f?"•+¨¤?@yQƒ–†'?wæT¯Eø?{ÈC°?îÜö·gïr?‰kQ­¾d±?b'œë¾Š?Pe†§àõ¥?¡jºÅ F?ˆ­—ç	û)?ï?ØÛ$õê?€-ãAzG?Eªtv{>?8ÿClxõ!?—W÷°ÆÝ?€+мCÙ4FGL J2255.2+2411¿ë·MYؗÀ?ˆ;`(^ÄÀ93´±M†À<IF"@n[4Ùü`@Ûª€qªg?¨àA¸uí¿Uäa`d'?±¯Û @Ê! c¸6¿áþ3a¬Bi¿áNË?.¿â<8*ù¿áŸà¥Ç¥F¿àßÕó¼ûž¿à&JLTliAGNbll3FGL J2255.1+2411MG3 J225517+2409?ï˜ÿ»zË?…¸ˆ|À"?DÌϵè.?>ÖE¿ï­?ˆ®3ϾI?…"Þxín?Þμ"?•½-.¹?7š^¨}v>?Yªë<1ž?Šb5W
á?"'YÅù?îÒ(˜¨³¡?‹`1þk~©?pMŒå(î§?f	'
E}U? ÓÄØϨ,?ˆ°Åh*4õ?ïmèñ)IÜ?|ëìv¢?`Æ,Ý:À?R\‹¤G?*?/lc?yú¼E_T4FGL J2256.0-2740?ï«Ékˆ(ÀPýŸÓo~À9<çƒ1xHÀ;Uù†i;-@åBÕ<²ä@¡…÷%f?´f~«<ë?'Ÿ˜6B1S?ÚÔ֜?@	ðÖ. Qo¿ÝŒZ@é)O¿éÃÌÞj"¿êˆì9ò¿êŸ<¦y{í¿ïÿtN†v?ÇÙ府mAGNfsrqPKS 2253-278?ïú^¯Æ?Lu¯>œ$"?毻þE?""P-ˏŽ?D
ÀÁ p?IRH¸yR?f‹É?\ZMÄ:?P#ðÌ+N?jýoh'hÅ?†hC¶#ú?ŒOÜ¿§!C?ì›ø—çٌ?¤µN	4Ø?'Í¥ÍouÑ?Œ çP`?¶lÑÍeV(?¡Úx"BÀå?ïlÃQ(ª±?ƒ·Ö4tJ?VYY€]ù?PN>GáH?'BäÙ?ƒvghÅU,4FGL J2256.4-7119?ã*®JÖÀE~p\‰mÒÀ;~à^zÛÀ<âòŒyöf@""'y´¤?ó§®ë:v?ÓmJ[BñÂ?Ûpmü1ê3@ ÀŸ—à\@õƒÈ!{?ïû¼PíX¿æá¨&$W¿ïÿïXz?ïÿÝ/ñ_S¿ÖA9†3‹H¿Åüº¦.¨_AGNbcuPMN J2256-7115?ï	0jp-?›ŒóMHÓ?luܵº\F?j'gï"?›Mž[ú®Ñ?šA"×'9?îó_Ρº1?¥¡G¹}
?m/Z÷Ìÿï?"ðWA}?îÌϼ?¢{5{û?ìœzóOÁ?¡µ«	U7?ˆ:Á铎H?|fR›Ð?¸Ð*k-? tím³Ù?í˜ßÔgtB?¦ö•ý[Ó?v¤¡'wç?…k$þ¾·?±Î·C²vx?¦Æx'µÒ4FGL J2256.6-2011¿è¬'ðˆÞÀOr" ٔ[À9cÑû	öúÀ<1¾Ûrþ@Ìâ'q	@À5¤'?¬˜ßàOáj?šgà9B?íñg™T@D
ájÿà,RÚš¿ßECÁu֜¿ãy î?
¿ÜEíhMÇ¿æƒ_—±¿äiM š)aAGNbll3FGL J2256.7-2011PKS 2254-204?ìwcy,j?²'5 +q²?pVMœùí1?e "™V?»AÀ
fýÞ?²[•ø
:?ﲈÔa°?¬2Ýñ̉?gØ^ÁPB?Pž;^Ê??œn£
R?õ?ªÞæy?ë2ù\ù\‰?¦(xƒDÀ¶?'Ú0d¾)?T}œm?ÀøÔ'ȹ?¥çùWýƒ?îVl÷\Zu?'B©Ó.B"?†°%²?u =?Ôz?¥/^1	?ŒõÖ&Ò¦4FGL J2256.7+1307¿ïY úO֜ÀDˆŠÅÁ@À;~d^NÀ<5·qñµ@ S‡QŸ¯?þ+£!h0?ÐKÍ=µî?Á•Æü(Z?ò-žž¼J@žx±A«ò¿ÞÁÍ_™Ã‹¿ÎÀ¸Azsº¿Ø«hC`Qú¿Üö)RáP¿àVÎþÖ4U¿ïÿóÀ¬ƒAGNbllNVSS J225624+130541?ïÅ="ñnL?mÏ#‹Z?9¼'—
 ©?2…"iøÃ?{Åtm×ÿÛ?léYÒsY?ïPó[?š?™jÀ_nͼ?OÎI	ðŸ?^Z/·SKÇ?œ·oLP?˜}Á%è1t?îQZK2?è?†ô{¯^Ô«?q÷TªÏð0?bê2ïÝΎ?¨«p·'v?…éÁo´?í¦Ç…Ž5Í?yÉICOŒ?a Ã8ÙÀ?T½;ŠÙÒ?²<ýtŠÒ?eþWä!i4FGL J2257.5+0748?ÜS¦‡áÚÀF¿ŒâÑñÐÀ:֟vRl´À<n¡¾+IZ@X>A¯!ì@'ìCŠ™L?Я¢šÛ¹?¾1ì'9ÿ?æÕL}‡\@«QȽ/¿ç8"Üû¿çwk§^¿ÓàŽ€`ãp¿ç͑¸ú‡ñ¿ïû5`4>?¿¦Þüz9'AGNbllOY 91?îâ#Øu2N?š§a~<ž9?X^T8ô@?V4ñõrÃ?¡Ï×Ët?š"õO¥™s?ï4U)þ?"V"ýßÿ³?RªšÆržº?aþÓÒ¿™y?˜R+³3–E?"Pj.	?íaZ¤
Ëe?–@öõ®ä?'šØgö¾M?"òsñQO?°Žtœõ;?']«ÖÚÌ?ï
ÊÁ`?'$.€ ²?Yñö¥<?N¬sp±?ˆrƒ˜Á?àVÓC"4FGL J2258.1-2759?æçüýRaÞÀP;0"'À8=RpæÀ;Sß'Bd)@ ÔûðPà@L…0aÈ?¡€Å?î?ÉVEÜÙ	q@#–žš@¼à€ø¿µ¾!Á¿ÛFËÿ€¿åM1:Æ¥¿è(bTˆîQ¿ëOý¤-f¿í
òl™†NAGNfsrq3FGL J2258.0-2759PKS 2255-282?ê*1Ç?íê?¿ [ÿ‡?¾¦8ÛìW?®B®'ƒß?°yn©C›ß?ï?žÓ¦'?¤-Ýê?iXÉa[u?‰1ÏÓ¥¼?"é,_®?¡"ÿä-<?çð"—m¶Ï?´(a§oÞ?ÃTVGö{Ó?®"()0æ%?¹Ó.´¥Që?¨(«Œº¶È?ï;šÝ¨©þ?‰'Z-è?g
ú ß??aJ€"wt?•«DöÎØK?‡5Š¸4?ã4FGL J2258.3-3643¿æ1ÑuöH¿ÀP*0U2aÀ:–…`ýpÚÀ<¥šàÁvW@V¯ÂÐʈ@š"ù$D?ÀlrYŽ¼œ?£tå㧸I?ãm­¸4T@	9Yèԕ¿ï`ƒ-FŠ(?ïòI~N9Ÿ¿Ü)ªu[Í¿éŸKT'(Œ?ª›ÈüfK¿èW'[åYAGNbll3FGL J2258.2-3645MRSS 406-025483?ïçÔâ!ªF?`‡w‡Û?;>q†,¿#?5–‰ŸëÈf?dÃO­#j?_n•P¥
?ï×P>£-?yÒ|=81?$XˆªXó?D\ GTj"?sµiµ¦?xÕô¸÷ǁ?î¸ÆDäÚü?ŒeÜ+Éh'?rîâ>Ënk?lE›_Èc?¢¿iØâp?‰Å²m0!?ïÑxŸÖš?b"Ú½Y~?0¸
T¼ÉB?-	ÛÅÆ3?v8/?g4o?bN^*'4FGL J2258.4-5524¿ÜçCÛ÷âûÀK;Oag#À:aƒ3%Ç:À<¯
@Ë¢*@ya¸âÔ@(a´Oþ?²ÓÁž‡Á¿¬§i¢Q?úPŒû%¥¬?ÿÐÈLŠr4?ÄÍÀ"!¿çÓ²ßæ¯ø¿ãÔ%¼R+F¿à"ØÅ0 ¿Û]:É)ª¿æAž¥AGNbll3FGL J2258.3-5526PMN J2258-5526?î|Šð"?šàܟњ?~uúք·"?t=\c!×?¤pGö.ß?™]{ŸÚó?ïû!ùz?šIvU῀?\Ž&‡|À?eúaE-ž†?­sIƒ?™A>¢u?&?ížg§£š?'"ÖrÎ	?ƒ*±Z±^J?u\HB¬'?°§l—'·b?eä?îpïŠ|%?‰B» œ?'ߢª½?p¸H"ï†Ã?¢/Oo"?‡[:À¡ö4FGL J2258.5-8247?ä̀
É©úÀ@¶ YžØÀ9Г¯tÍ1À<4‹ƒVa6@*wB+ɇ@¥ ¶Xí?»]7ÄB?ç-@÷Ý@A¶Ô=—@:«C:<g¿à.'à¿ÙÈõ<WŸ#¿Ú!(¤c÷÷¿Ý{ñ½òêC¿éEÚÍa¿ãdeጢAGNbcu3FGL J2258.1-8248PMN J2258-8246?ï¨ùd^8ª?£ºe½
è—?v~8y†p?–ø&žÙ¶?uÌj%)?'4)ótáG?ï\>7s¹?"¿Y-鴊?Q ãÚt–ô?d"§w¿ÇŸ?"b)ûj?O?'R/Ü{?ïÆó—?ˆR€Ð±œ?wè+ނ;û?zÌÐõk:?™-¤l,?€‹.r…e?îj
dH?ˆ
â[8>Í?Ú ëV`?jäZTÀ ?¤çÇ$C5Ý?†uÿ¸¹Õ­4FGL J2259.7-3549?íõ"À³SÀP05~gÀ:zj]këáÀ<•ýÉÄÛ@ì&.6Ÿ@ewmÏ?»¤ðñ4‹¿"ž/aê›?ØñOƒJø¢@žëq}›·?—¿¸€ÿ2¿¿èWï«&\¿æ>´`šI˜¿×wR|¤–M¿í þG™ſĒ©ei'>AGNfsrq3FGL J2300.1-3547NVSS J225941-354846?ï)avà"?'—Ô )ÎÖ?q7$>V?dª—‡Lh%?–†É°?'J!<üV?ïµ8'wÿ¼?…½í¤Æ'y?7˜ƒX9©É?QxŒòË?õG>Cö?"îJù±û?îKºœÁ1?,¡nLž?ƒsñ
þt•?~/á~©N?¦gYðg_Ê?ˆ"+̽¨£?壟_^ß°?m}Öֆ"?^²â;U?N—Fàî'A?'ÍQÌLa?jõÏdwI‡4FGL J2259.8-1552?íZHTâíÀNå‡?úÁÓÀ9ùqÆùgÀ<`9»°è@7/
.­@DJ9ßõž?º+œk[?ºÿ"JOY…@µ­é¿@b?Š.˜¿Ò¿žÁ÷‡¿ÜÂn$ïß¿ãbåþL À¿à®°³ ¬¿äŒñ_Ô&¿é¨eå7&ÞAGNbcu3FGL J2259.9-1553GALEXASC J225957.26-155332.5?ï앗«ÿ!?TM1åQÀ´?1ÁÊ2¥?&¢©Ée5o?a2HS§™M?RÌÞDüÌÓ?ïÑñ©¦žl?|™ï|aoî?'­¦¿FF?D ¯µ^‰X?vIzÏc?{¤¿éý>?ïUŽ¦"D?w´:Nè5ô?c§`>0¹Z?U›OĦ‡=?'ÙSCg€m?uág†Ú.?ïÀ1™Ë!×?aØâÂü"?Fc‰gDÏ1?3Ë©¡XÿÏ?}Áí†{[?a>KÔ|KÕ4FGL J2300.1+4053?è¡‹wå6À1=³(é-À;4½çXÀ<œIwBV½@":QŠŒ5ƒ?÷˜ƒ$"?Ó¶, ð;?Ñ5@Ԇ€?ú…dÃÎ÷I@õ˙Fª?ïpŽ• ¿ïúS] ;?íÒ ¶ÄLÌ¿¸úÕ^@Ó¿Ð9*ƒŒ<¿Ù?͚'AGNbll3FGL J2300.0+4053NVSS J230012+405224?îļ˜ðI¦? ˜rP²?^~­$âc?[½"ùi?¢ÃÚ{'>Ž? C8•ý<?ïEØÝí?˜ÅŐåÏ?QFÝàð¼ý?e75£Ýë?–0é}6?˜ñvCáä?ìÞwe%Ç?Ÿ5±w¦8?xŒÜ/4}Ó?kž2¨&y?·ƒy©ã‰í?žYú0çæ©?ín½]¿n?ž?ÂSúÎ?T3<°c9?PÞÔry?´9HÉÎk?ž"Ô±O=4FGL J2300.3+3136¿ë4´döúžÀ9'ê>xâÀ9'üaåÎÀ;øV"ŒÂ@d?3F©]?ûÀ§$œ—?´(Ùþc´?Ãï$eü¸@cÈ}²³F@Qä&?ïæªY~?×êdbU4»¿Ôòñ#Ä*g¿Øj'ò"È¿áæïÃqÚ8¿èŠ.A±ÑAGNbll3FGL J2300.3+3136NVSS J230022+313703?ç·ä¶[?º2Ò|g¡õ?ÁWQDÁÿì?¶8ý™î&?¿'7Åë½N?®SÃt3ÿ?çþ$Ö3~¡?ÅÓ´¢Ë|d?½z)/ö•?Áúîj· Ô?ÁJX6ºë?µCÅŽhÇ?çÁ¶ö.s?®€ï¼;@?ºW¥@ös…?¤	"¹srê?ÃÍTó¬u?¥
ÉO$ih?âÝî.?³
ؤÂK)?¶	"ïë?¡"â-Bî(?ÔÃ`àçÌÜ?µ¹HP6›Í4FGL J2300.7-2645¿å ³ÍnÖÀPWæšÔ,=À:ݲ"ý[
À<{k%@áöfÏÿ@i=¾§p?ØOsûÐE}?ÙNäH•@:ßdš@Næ¤g¢¿Ü÷K%˜?ý?ìԝ¡;#˜¿â~\&qƒÑ¿ä‡ä€G¸ü¿ïý~E€<ѿ䈴€ÈAGNfsrqPKS 2257-270?ï¿X>·–?u£ŒŽÈd'?\ðóVö¿Û?X^­ží~?yÁ
慽?sb¼M¡b?ï–
A­4?£­ýA?N¦û*ÎM?dœÂTŒf©?ˆŒüçÎb?Ž})è¢óö?ìø,ßIÈ?œ
H"°1'?Ÿ:"؁ˆ?ãE•ð?°o÷þ;žÚ?")fþêJ¥?ïXid=¹ô?zÐ{=øx?Y"hWÉÜ©?Q¢ó6'¹L?"YŒòÌ#Ê?z,'ÞÚ/4FGL J2300.8-0736¿³ïfX±"ÀLªt)ˆ<À;1²åšùìÀ<¢f®ŠÂf@ ÔÏj5þÀ?ÿ:o¸¿ß?Ã÷¤;Þþ¿§öO¨ó?äëûѝ&?û²{诿ì,¸Å®ËZ?'¿FÚãn'¿ã®ÊM–‹È¿ÖÛt/|ÅM¿åÛ;à€Þ¸?Å£3÷(kAGNbcu2MASS J23005469-0735438?ï¡]ov—¿?|\ß	¤È?ApŒm?í?4vÏO°?†˜-"<N?{âY£+y?ïaþºäã?'|U`À?NwßÜ?›?YÆjæý•…?'̉Áfº?"º– 
?î;‰£s["?ó€-~¼q?p}(hS|e?\=¶ÅÁF?ª7À»¿Ø8?Ž[K<љ?ìá¦{[…»? ~åÛùK?tó«aW™?iޛqEjf?·£'oX›?¡°àåÆ4FGL J2300.9+7108?Þ)¾í]ˆi@$XNaŒâÒÀ;B* dúVÀ<¡'~Ê
{@ íœøž·¼@g£Àd¾?Ö2%™È"?ÝMŸ$óÕO@0K!f'@F2"QÜ¿ï²BÝË!Ò?æ÷,Êx?ïÿ×ñÃý¿Ú°ïáú±b¿ê\Ö/Læ¿ÚgC›‹6TAGNbcu87GB 225907.3+705409?â·v—U¾r?ÈAjÌͤ¬?´7m'õ)?³ý‹h܂A?Ճ7Š
…Ñ?Ǖl³Nò?é+SÞ$K"?ÆìZ‹Ú?¥PÒ§®	‰?ª§#iE?Åþ{݃Q?Ä5êý"&?èÌS5 ?©ÔÉǸ?²ŠÈø ×š?™°êȗl?ƛj6Û5?¤P6sˆÄ?é¸ØA¨¡7?²-=Yln—?²Ìe!íG!?«Ô³}1?¿lØÐͯ*?­ýÏs5W4FGL J2301.0-0158¿ì¡ÉšïÀJÁ—¢H"ÄÀ9KþmuNÀ<͆00I@	('Ö¶@ˆ+輜?°ðZE›À?»{u·O¸@S;wG@¯ga8)¿¿8¦³³v¿á垪Ðy¿æ½}h5ž¿æ†yKD!¿éïj¼6|"¿ïÿîbHÊtAGNfsrqPKS B2258-022?ïÕô.Îá¯?lú­èÖ?BUüøÖkâ?8"(ŽV?r»(ùtZË?kÆiŸéØu?ïÏG»Ù(?|­Ò_'˜?0`üðÚ«¯?QŸ×äMM‡?wVD^GŽ?{dÙÞ·u?ïrEV‹5?€EIž˜<?p¢_X¥Ì?ZóIk8"?˜IS	?}é¤bÏwÃ?ïíA~uH?Makf¨Ol?#ßÍ/òÜ»?:ºÑ‡ËÃ?a€"·ëŒç?K×E˜ùø4FGL J2302.8-1841¿Ñÿ‡"ßJ©ÀO×L`RPÀ:»¸/†ÖHÀ<¡Èê¿üÛ@ªòêí¿@ä"]?v8?ƶgZ­³?­1÷㕪æ?åÌÙAÐ/@]tWjÊú?ì!ÙzZ9¿ä¿'Bd(Ÿ¿àüö•óò¬¿áï;â"D¿æZUÖ¿ïÿo˜AGNrdgPKS 2300-18?ïu!¿·™e?ºîãh?Z'ŽedV?O\2k†×\?tÝàLùó?€á¨xÚXü?ï{"Üà
?<Ážg¼?Jü—Ë—áh?[¼»¿MJ?nÿ'Ž[?NÑv?î$­Ì 
?›grèèÏ?z*D˜-2Ô?iüŅÝÒÅ?ªoÚ«ØXÓ?Š"öˆñ?îš5Ë?U?"_ìuÖ?qh›¦hc¾?[–›ëTGo?¤/×=š?"#Áô`ºd4FGL J2304.3+0618?ì•ëÀGÙmã2iàÀ:¢iÿxÄÀ<`FS¡gÄ@¾
0•5@úxCÞ|"?Ï0Æ[ïj?ÍGÇêºÉj?øc×ZÅHt@
å+|…Œœ?ïþ~ÀÐ?H¿áî÷. &|¿è™¢¨áá¿æð(A<¶?¿ïÿ¿h`;ª?ïZZ¿i6ûAGNbcuPKS 2301+060?ïäHX/÷˜?j/Օù½?8Vû戯´?8ôÛ0\ái?h¬ÈS7R¤?h:õlkëø?ï:'¥,"?™Ó™'ɘ?Zœà|é~¼?k"pÐhþ¹?—‹×q?—t—ŸÀ†~?î™þõ€o˜?‹–_<w{?T^U+?r¤'Vç	?¢~†.V{?‡|öE¨?ï€SF"¬?vI04iŽ^?YoÕc¶Ã?K¸¶Œ"Â?ŒÏðû½å?u?ÉNc÷"4FGL J2304.6+3704?ïish}À5¤]AúvÀ9"n"2QŒÀ<XÓÖ¬@ TÐó"?ýpoiDg8?±—÷-š?}ÅmáC¢"?Íè¤CÁ Ê@
/¬G¿»¦æÿ(¿Ûl¢ Sr¿åï¤"^¤¦¿ÍEþâô¿ÔÑ{ˆ6šÇ¿Ýá/ÅÀiAGNbll3FGL J2304.6+37041RXS J230437.1+370506?ïò®'j?Q:Á¡–r ?øiæ/Ç?dƒÝn'™?XâTÜÊø?PT"ë²SÛ?ïÛñx#­ ?uï~®…î¾?"BÚ,0:o?>{øcž7?qu-Ç®¼?uTT:æ.?îÕº
)?‰˜û#x?bëhöÛ§[?T¾I[ÅÚô?¡u¨ _µk?ˆþ#v°Ú?ï­Òh10?hQ¸8Gß?@Ezu©ÀÙ?2mkl?ƒ‡W™?g³uáÉ4FGL J2306.6-1105¿ÕÃÊOnþÀNMêhìSÀ;+š8ûÊÀ<¢RÃò2¸@ü%4ÂÕR@éĤà¹?Âìv¶?Ž¿œ«ÒèUûp?Ü}Y\'¨?þdÐTÖ×?îI±Y¤·?æ*¿ëò¸ࢿÙÅ» 'è¿ÈO8·×rB¿æ®"2Q‹äAGNbllRBS 1943?™)A	?¦pÒTv+?c•¯d7¡·?^ÆtxŠ¿$?¦,Ûw(uX?¦
F-C?i (?!àLÔ¥ ?EõcÄ©8?S	nÍ¢¬¡?Ž1Ï{«bì?‹úl)Ï÷ù?í~ú0L?—X7¥:å?v	´à8æÌ?cÄ0?²§"/œ¨?–Y͂¡·'?îArɤ,ß?'ï{pp Á?q§¬X?jxºHý%î?©³áÂç ?'­-|Rö£4FGL J2307.4-1206¿ï2ªú¿ú+ÀN°µˆãhñÀ;JÅø5À<«¤¸²@ Î
ŽÞՎ?ÿCýrr
?ÅGQù#¿'ŒÛñH?ÐõêÓH@Š‡À©(?퓿e=W?áÅÂíOú¿â¦ìq­Â¿ïÿêf:Ç|?ïÿž{€©ß¿á¨Ðº%*AGNbll3FGL J2307.4-12081RXS J230722.5-120520?ïáýêül?p«µÝÒ-?-žw±µPó?.÷çì-(?l(-ˆx©¸?p†Y–]ó?ï®';Ó?—Ïǧ§E‡?Tñq. ç'?t0ÔfëC¦?vGöÜî$?"<÷ÈÌ8?í|…F?"ÀÖe¶_?ƒ#&G™Þ?€ÂÆòo^<?±·o2LÜ?'ð»z)_?îòîªC‰?•pdú¶w?/2éÒ·ÕU?7b{§H¥L? ¸®+‰—?•r$ÂÖúM4FGL J2307.6+1451?är#ó>|ÀD…Å3À:!ó¥~ª*À<*¬3Ð%@AÎ\
m?ÿä̝Òä>?Ä;9ýQÏÖ?Ì
ɲ'@¬Á^ڀê@G¾Šß¿çëi~J‰¿ç¡ŸÒò¿Ù:€™îS/¿âßN_¤¿ä:aûš°¿é{bŸÝVAGNbll3FGL J2307.7+1449MG1 J230734+1449?ïÒå,{(?oJ°m™^Ú?Q>]‰ùòû?HÖîr–öY?r=ҝCïÈ?kÜÖÈ+ôã?ï½õq†Úç?#ü«Uêm?*äwúïä?D©Ú߇ &?€¾a"@?€'»(Mô?íÕ«`r"·?š<æ»o??ˆ‡;+ě¢?€I³5õZ[?¬ƒ{-坹?–cWïÓ2Â?ï'Ï»"nB?t–ÖɉM
?>溥ÚÍ?1àÍ!"ñ›?ŽTÛEµ˜Ý?t]/ëÃm›4FGL J2308.9+1111?Çý›G׍ÀF)Q֌i/À:¥àªÐ"ÃÀ<uý'w>%@öª'».@(…ZGt3?ȎpÜ.1?Ò«3À ìà@3Äz@a¦ˆ›p¿ïÿúŒ—Ó?ïÿÄ}îB¿á¸rØd°"¿åVõ°å_¿ìnç©Çå¿°ûUvT4AGNbcuMG1 J230850+1112?îºRåí?›y¸[=—¿?~ªâ³tC?·˜ë:? …I"«?—z(¼É?ïsÞÅÉ?›OýÇ8ÿ½?b®ƒƒ°'@?t…¯2L?›[³Í4'?˜Sýüm?ì:ðgÚ?¡¯Hg'"Ö?¦²ÜÛυµ?"½ç;h?´nº"þP?—§¨¤ºH÷?îõé¤6÷Ä?2Bnr?wY¹Ýq{Æ?cf'Oø¯?›l]Ĩ"?~¦eô4FGL J2309.7-3632¿ïP¶)$ðÀP¡¸€®À:&AؤmÀ<rÐîš}@Í;­*E#@,™»þHp?´ '§7¿•ye»Vê?áìi ,°¸@¿­QÝBf?ïþÖj€˜¿ä\º:#è¿à5ŽÂ¦^¿Úr¼€Nnù¿â'—|ˆç›¿ÖàÀ48ñAGNbcu3FGL J2309.6-3633WISEA J230940.84-363248.7?ïoÒïęæ?'»Y‡–'?TÑ5G•?S
""Ür?¸†	nÅ?µ¿ä?ïuÙ`…¸˜?'ú§Çœ?L‰†N
ÿŽ?\"–,¢?`‡¼Ø} ?8¬he?íkž–""?–"Gêâ5?G¸kÛÿ•?qDb]ø_?²z=çßÞ?"±ïÍóM?îF)GýOz?Œÿ'ÎÕú?vÌUNƠ̂?cêo‡Úh?¨ÃàÖPnà?ŠÞö¶ì)4FGL J2311.0+0205¿æ"Æ`÷çƒÀJºÇË)À9n‹îNÀ<*ÀY!†@O²(؇@Üðû?±'®*?¸UW༘Í@HçÖyõ@'~k)¿å•XA_›Ç¿Ê1V?Qпâ*È˶LX¿çy]ä☿ߺ?<¿ë…Ð>qT×AGNbll3FGL J2311.0+0204NVSS J231101+020504?ïÜÎ<¥±Û?fß·À'–?*sâ
/ªô?%ºZ™8[?pÅBœ½"¥?f-ìòog?ïθU4-!?{·Ø\ß?%ÔìŒÐ@æ??‡A­hKð?wõ.'î"?yÿDÌá‰?îβÅ1Î?Š'"å¼Ï?xôÂ׏¦?s…âù"ˆ"?Ÿì‹'™b_?†ÿ8 5ç?ïàMå"Ñ?Xèfa浌?,®s¿ª–? +ÆÁ"Ï.?mèÞ{Á?X)Æm°4FGL J2311.0+3425?ïǦ*TEÀ8煵·À7Òv pMpÀ;žq—òÐm@ò E>y@ëDå^³?˜lð÷¬ýØ?¸YaL1‡@nƒ
áÛ@l7ñ³áï¿´º`
±Ä^¿àÈÊ^³i¤¿å˜9²©5¿å&[^u6¿ë¡ê Ðâ¿èç=@Ó.çAGNFSRQ3FGL J2311.0+3425B2 2308+34?ï¹N6‹_#?uÉåÖN ?\Èî­`Ã?WÊ<ú•?|&©–A?s¼ð2sØÒ?ï¡8ppÞ?‹ÀÍö™?EI2ºË?UŸ¿j¤"Ü?†fÞ¸B+e?‹:¢ÜW~µ?î[É¡'˜?šºP‹'?"¤é•Á_Ï?JáÈT?ŸúÝ6M?"v¦€(3?ïõҔ±Ô§?F"Dõª3m?,p–'–Ó?''0¬Î Ä?PÌÃؤb‰?Dz"Ÿîü–4FGL J2311.7+2604¿äÿ¢¥0üwÀ? ˜€"åÖÀ:)Ö¢8¤ŒÀ<Sæ
ær@®¦xÓ{@!§ýàk?¼m<ïI¤d?©ÍáʵÆK?뙟}^P@•\Tê"?펄'¡WÔ¿áPž1Ú¿åà iA¿åé¯nî¿ä¯^'AcM¿ïë»MlšAGNbcuMG3 J231144+2604?ï¡oÜ'?€¨x@Ž˜H?AðT>µ?5tLèàۜ?†…6H"°B?€Pg\ið?ï¸ú9z'?'_û'?(ì1D@	N?A>µó1œ?]ÀÜN{ß?Þ	胅C?ï'À-4ß?|Êã],g??jW˜Ši?U¼!Þa›?—½Êh?zTÕ9:¢4?ïªe°¾?bë]DŠ?Eìa³#úx?3¸Ì‰kÌ
?|A–Ã!Ð?b`Ñ+Èã4FGL J2311.8+4541?°¸Èx0;¨À+}´í²öbÀ:ˆþ{À<4å†×õö@»›¢|@|ôètÉ?Çï­7OË?ß"š‰®•?÷ï~Þ,p¡@×mŠNÎ?ؑÃâB׿âÈñ EØ¿êI
Z[–)¿á1‰Ÿü_7¿ïÿø]Ê5™?íÕx™]4AGNfsrqMG4 J231144+4543?ï	"Q¦œ?"»³?'	?ƒÚ¾{Qô?¬bޗ¼?"àgëò#ˆ?JÚ¢s]‡?îÈÏai—ž?£z\;!é?qvªâI;?'Ï™¤eE?¡D4dº?¡Nà'{;B?í!߆0B‹?š­ï©ŸÎ?‹ÃÞÖ͛?zä—V«»?³«R£ß?—SΟ$î?îJö ñá†?ïM@HÈ4?çüx·?n8»Àv©?¦ÖØñßÉv?ŽöþÏÿ=b4FGL J2312.5+7241¿ê"T¢]|L@&xaՈÀ:Áñx}ÀÀ<4^[Õê@Uyqk'@{¹Fk?Ȗ³á‰9?פõ'Î{ù@¶l£—I]@¤Ge_M?ïÿï9_J¿ÙÃSÜöæ|¿â§§^~:™¿æ……t¿éþ	ù~¿ïüÓ$Õ¢^AGNbcuCRATES J2312+7241?î ÃdÙA?¦Ã9Ó>W?y7à-Ûõ?u5Ÿ¬?«O­¬°ˆ?¥y_ÓÝû?ëãïÀyø?Á(6ðKk"?Œù¡h´·?—M

:Îå?½AMÏ!5†?ÀG>Ýó9?êi³á½­?¥8"'ãf?¬)MðÊÛ¾?"iy4–0?¾¹ù²4·? RÈ ë
?ë;§£ÉÓÕ? s`ŠÕÛ%?'j+sI?|ùè||å?ÀßÀ"BE?ž«µ¿2ü14FGL J2313.4-6922?æÍ¥d>:ÀF²SCsóÀ;Ÿ]ZN*/À<ë{o'V@"³u†iæù?÷Ϧ©?Δm_ÔÑÔ?ÍG,å;Xœ@>;¤ò@åÃèL°¿íu/¢/k¿ÖB²A±%Q?ïü÷"
í?ҁüœÌ¿ååwÞ³Õ?ÓPúïIúAGNbcu3FGL J2312.9-6923SUMSS J231347-692332?ï¾G.QÈA?—"ÏquÓ?Cz[2)4m?bàn®E~b?~mpÖ¸?•Xé3«r?bŸKÒ?Œe´U4H?>;&^¼Â?RY‡‡Ñn-?‹lN%7'B?‹Jʹú ?í¦íþ×?š.ÿ^tÛ-?mbj9m•Œ?c7µ6?±Ýƒî=ړ?šN…ÑÔe?ïYG[¥²#?"E{gø?Fо¾½ß?Fدój½´?" Ž•SÏ¢?ƒ®œB§4FGL J2313.5+3945¿ìÆ[žâ-ÝÀ3U<¼M#À9³¨eå7'À<!ܘòª­@½sßrl@=ŠT'8T?»òÂ?U*?ęÎØþ´@¨«ÕÜ@@`äƓ¢µ¿ÃÔ¤¯ò¿æl{=ãæD¿é¬MÑD*Ò¿í(~#qt¿àf6`]'¿ðAGNbcu3FGL J2313.1+393587GB 231102.6+393314?ï÷cÚÈÚ?PVýÀº˜?7½Zu)öK?7"á"eN
?F'ê®G?H-$…E3Ÿ?ïÉG#1}l?'/iUp'Ä?7¦/îHږ?X·,])ð?yâh\¼f?€Á',ÝôÓ?îÅóµïË?Žó…Oî?wªï­Tž?r'ÉÂB? «f°v€?ŠÞEÌЀ?ïÖJPgl?_$†àì:<?@–:µE?4Tx\Zt?rÈÿ¤òù?]`š.·4FGL J2313.9-4501¿¼Ï£ä¹ÀOÊìë¯À:R€;$À<FÅA¾q@½UzþÂ@H.D¶é6?¼/©Ýˆ\?"Ö^úiñ"?ÐD4¢Éî÷@dÕcIP¿æ"G!ý¿ã?¾&@Üi¿êù­ ·›¿ëÞµbLü2¿¾"V7$¿ðAGNbcuPKS 2311-452?ïçݽmÝ}?qC—ât>?LÏÿ^¯?P/}3$®?`îBˊù>?o6Ÿ¬­œ˜?ï¤vPP¯?"€|ûNô)?C4ÃYíœ?gܾFÒâË?…¯+žž?'š‰Q#´?í±äê
fO?™Ñ[¬‹‹g?|mpZÁ¬‹?pm•§P~?°ª©è²³?˜
ZÞ$ƒ?ïЁµ0Ò ?hò±L©?8"7ÅsÐ?4;陻&—?v5áõª™1?gt-:Jê4FGL J2314.0+1445¿êçoD¨ÈÙÀDôsš¿À9¶L¨O?À< >ÏH¨@ ajNÚY?ü¾ú1‰æ?µίP7?¯Ø\"Ó?û½CÂÍoŠ@JÆ!âÔ¿Ø°îŸÛR!?â盺Ü	¿ÞßÑ ïcÑ¿ÙT)McÓ¿ÞþGï¿Ö›;$™<}AGNbll3FGL J2314.0+1443RGB J2313+147?î×ï«°?"0Hè¯Á?d0¾6x?Z)h›õðÈ?¡72Mé¬?'­²}ò_Ÿ?ï4î#L-U?"ËL¶>;j?Wzæ3?e‹rp¸U?—ðCõiÆä?"rS^!ç?ìó~ds#U?3P®®c?…;ñ¹[m?wãÓÛ([?µ¼ª¾/¹â?™áÄ·"šä?ì©!tÔJ
?•‹[Üý'ü?…оÖÕy?pŠãž÷ïB?·üÜ~™õ?",A#¾)Ú4FGL J2315.6-5018¿»viO
:}ÀN?Žâ†ruÀ:3"_ôöÀ<zäÎKR@×5›J@N_œGÉÃ?»ÐßoÖk¿B'Â%™?К©#¥K©@=tю'¡¿ëåN¾©ô[¿Òe­ÄHﳿæê~Ž{X¿àµâoÌ@¶¿îÌaË¡ÿ?ÏÁ¡
&I–AGNbll3FGL J2315.7-5018PKS 2312-505?ïÂ-¹è¢?t¡ŸdUª?KêuéI?@ä
{¨™?{káNN†W?s4J3-Ý?ïÜz>†z?yG—?žÂ?"-Ý~OÍ+?C.0¤~Ó?q1qÐÐt?xA.A¤â?î¾óDJc?.ÇjjŒ?ƒn·´4ü~?~㫑æcY?žj;¥Ü5?‰šbD¼[¯?ï蓢ì±C?T4ŽnE]?6aþ¶Üº?+ ÈÎvü?d <s%o?RÙcÞ÷Z4FGL J2316.9-5210?Ój`ДoÀM­ÝiÓÀ;)û¤P¬ÁÀ<ÐÄe¨Ñ@ T
$Ç	¿?û¡Îl	=–?ÒÑE= ó?¾ùÝ?û\q?çt/è%ç?ÿ©F«
/Y¿æ5à¿ék×3X¿ã¾+Ÿ@!®¿Æßjßÿã@ä̝Òä¿Ú½†þâHµAGNbll3FGL J2316.8-5209SUMSS J231701-521003?ï£äˆ‡È†?yòWFg?8@ä~ó{?1
Ò"±€L?†DÖ½éæÔ?y"ø¸0S?JƦb?ïõÓò«?A"·
G!É?RR¶@=r?‹ÁÝõ±?ŒÑ¹Zü?î>),(?‹žMÙÖ¡?kèy2Á:?VhõÉ@¬?ª^å­ªR@?Š]€Gºý'?îÔ{Æô=v?†®µqë?Q$­ÀȈ?Guú¯3­«?¢/#N"g?†jÆSH¤4FGL J2317.0+3756¿ëoߣíÀ5GvĂ{pÀ:ĚŸ˜·À<K¯)M×#@Ñ·gµÇ@AËÚ^…Ç?Ë´ge¿Í`?¶­¾,0
?æqËtÝø@ížÏ
™Ç¿çæüÞãOƿ⸝Ö?<V¿áF%žu "¿æ°Ì@Šß—¿ïü•aütZ¿ï¾áÝU03AGNbcuB3 2314+377?ï6E:ø?Ÿ€Æª>?X€Ô/°â ?Vðø@êL>?š'*½'ç?Ÿ2NR`wÆ?ïÐÁÑÝ?›d`Zh÷l?^0…*1?mj%¦™QŽ?bßs.s?™¾±Ï+$b?íl#&!?—õCÛà?ŽŽÍîÌ4û?H7óN«•?°Í
IíHR?"¥ó©*?íÆÃWdÌ?'­À[p'L?u5d»?dÇÝ¿·ƒ?°x3'ƒ^8?' Ù|…}4FGL J2317.4-4533¿îD´° nµÀOâI@¼À:/e‰Ç"À<Vè³³ @½EªI6?ü¯§r 0?º2€…Ì];?ÆǍȪÿ@'3@˜™is?ïþ.~Ãq¿à2÷~|1Õ¿ØTü܊%¿ÝTVc¹ã¼¿ã~¬ãù9<¿é^­'*AGNbll3FGL J2317.3-4534SUMSS J231731-453400?ïÙªÌîª?hÅô2&Ë?X›äÑ1s"?SåPâ¸U?j@©`8?bßðë&
¨?@Ef*?"aºJÄÚ)?UŸaî^»2?ug	™'a?Œæ°Úž?ƒß:§‰?î³ÑóëN?Œ¬‹È¨Ä?…ò÷*…õ2?€B'^h/Á?žŒcŒ?›Ÿ?ƒ÷@®: ?îYn
$î?‹DŒy
Žb?h»†ÿÏ9?Z1!"h_?¨Ýfo0¿`?ŠŽdè²+M4FGL J2318.2+1915?ï9z$‰LDÀC4t}€^_À9²Áo¡x‹À<Íê>y@ËO¤@I´˜c9?¶Ì—Þ-G?|¿ûûZ÷?Å'T,þ@,½£9+¿à\VbbJοæ–{(,¿é0¸.°¿àÆးø¿îE·Ï冿ïü;ºÁ1ŽAGNbcu3FGL J2318.6+1912TXS 2315+189?ï÷¼8›|?I7úéΒÿ?3J_ß/S?+•Pð@Ø?GjÃ-úf'?E2?-?ïɅ*°á?€ãÇÃÇ9?0—ù$_Ü?Lÿqi&E-?z3ù¬•I€?Ó	ÛÊ×?ïMŠàì‡?z;		Fǝ?nsáKæ]?d/™K0ìŸ?'‹ñ'¸òE?vãĦ×uØ?ïåO…ÿfZ?U FZ%£m?EQØHo`?9ç—Q?en¥Š‡ˆ<?R€™Kƒ•4FGL J2319.1-4207¿îǪÜë†ÀP|+IºÀ:uú=H_ëÀ<•æÉÎ@,ùÏdVÂ@.Øà×EÍ?¹oÛÛ£
¿ŠŽÈvÉ?Ñ«Dœ'x?ý6"y þ'?è÷Z_G
[¿ãmü\ÝP©¿à'Æ-Vпà…à19¿âW°ö­pç¿Ûâ H£ÞAGNbll3FGL J2319.2-4207PKS 2316-423?ïlpê"ú?…ðÐ÷{n?Z-z>è?L°cƒ$?Ùº>̈Å?…ds"ý>Ë?ïSzöF•Á?";¶'†?Tðò?J´?_L0j[n?"A 8	SN?'?6¸?Á?íú
›î?¹¢S2?xá7üܵ"?f¹‡Dü9?­Cˆ&¥ˆc?Žýl^¾?íŽÉׁ?"¤Êä?'Ãñ\?m]Cû>?±gAÀï]Î?'ô¬ cÖ¼4FGL J2319.6-0456?Ú4ssúÀMkøüÖÔÀ:ü8ç¨fÀ<‰á<ÆYì@ '¦un?ú ˜ u?лR;Œ/?΅xdë'
?ÿ•S¹»@þ€G7w¿ï嵜.ŸP?ëýQÏÖl‰?•	i¤ù
¿Ð:n%wˆÎ¿áj3°0´Ô¿áI€|'!ÖAGNbcuNVSS J231929-045640?ï"µeÏ?~²R:5Ê)?S°'¢|(Ý?K[‡qØ<?ˆ†@rkÆÌ?}5 ̙Ùq?ï­8¼/Êß?†a¶Œ-Í?<oޞ–Lè?Pµî6‹û?ƒÎQÿ•±?…l\¡ë?í÷ˆþ[ï?'!ÔQ²J?}i—
€•?qaûKmza?¬àԎj.`?E´[ɏ?î¦w
éº{?†òbØxu?`Ç¡`G>?P_äcÏ?¤Œ—NSÙ?†…'ͨëº4FGL J2319.7+1609?سá[-ÀDªiƒQX¸À;/=÷²S¥À<¡ßòC~Û@ ¯´õj¥»?ùgk´"«?Òãk¿ì""?Ԕ–e¿ã@Á}ä1@düsÙk—¿ïþ›vóQ?ïòh!ýU׿垴‹g\¿¯>'iÈ¿á×U¼Ê÷
¿ïó¬ÐDÑAGNbllRX J2319.6+1611?ŸÊ? Î§Þ@?Rfšéçó/?F'6
0ùe?†IDáÐaº? ÑP²h»?ï–¶õâå?—ùØÇ0E•?\Z&¸0‹?i]‡qj?›g†µÀš¤?–q<O?íËJQÑ?—h7Õ¡?†h‹ÐØ·"?v¢Š½Ö™?°´"5*Z'?"{Ì3†?íJ›Õÿ`?—¬a'>é?ÁâD4g7?r_#&axá?³¯+Áµ?–4õþmÁ4FGL J2320.8-0823?æë7';ÒÀNőÙýÀ:Ÿ>ÔI™À<Q˜hA1ù@j×9bL@2Á¾{Ñ2?Û÷Ü°ožô?Ú+ഐ@@¹áåéÔ@	P§d?ïûU@¤4þ¿ä©ÅÌ'‹_¿é€¾×@Ä¿ë‡Làƒbö¿ïõN`¶#=¿ïÿ%D]'#AGNfsrqPKS 2318-087?ïÛYƒÔ-?nK»Û'™º?IUÐÝ­?Jƌ‡»ö9?nQ6â7šú?l*ó(—È?îïiÞÕ¿?¢®ZŠ#,?q›ߨ…?'ù÷¹ˆ(?«þírc¥?ŸÜ¦ý
?íuÿ†<?•wÀ|†»0?•7•íO}Ñ?"ÀñÎ¥'ü?®¥OÝO?¨ã«ã®?î<9(—?'½°‰Íö`?t'_[?o
`²S1?¬WZá‹.Ù?'!óqº*ú4FGL J2321.0-6308?»i—¸ÛÖÀIŠiƒQX¸À;[ìëPFÀ<îUsÏÛu@ ;òÈ	­?ýDÌh"ÿ	?ÉX°›>?À¤ÿ§j"?ó홖>›F@nr
—~?è¿Wߣ¿éì¶wò?³
|%js¿áMÚ~f7l¿â>™˜ÂÚ¿âw®aÐ*AGNbll2MASS J23203986-6309181?ïRǪ‰?‡Oqóщ3?RT"U8[.?E­`A'U?"˜Dê·)>?†ç‡VFA?ï-æY
£?•*Ô´±*0?Rõ5Ç]P?`Üø¹ m?™-2Q'5•?"I?'¢ûf?îì"'?Ž‰b[ ¨Î?pßT±8Å?]±Ûdì'p?¬ƒ»¦}?-³'GÚ?îAy/7%?‹ñ"¾^¬?k&†y¥­?\ÏRòA§?ª;ϔ¤ó^?‹æHTn'4FGL J2321.4+5111¿ÞêÅ
ï5À"hæŽ>ò"À:7{~% À<H¯¤Ùš@þI'¼1Ÿ@SüC²Ý7?¹2·ÖEœ?ha[¿¸J?±ww°»Ÿ(@dš´KÍ?âmy_èGý¿®e!0Á¿éõP¯Dü‰¿ÕXÅÉ£M¿Ñ¿

Áû¿í)\_§ZwAGNbcu3FGL J2321.3+5113NVSS J232127+511117?æ·ÂóC?Á9ڛ™pU?vYÄÚìP?iN.\fØ?Ò7¢?ÁÃJœ?ëÚ§#"¸?¿z©ˆµt_?9%!i)%?TˆåöÁ²›?À‹Jáá8Ž?¿`S6É"æ?ëG'¾È?£íu;K´'?†(Î^.þ?uƒÇûÚ²?Á€÷ü?¢Ñþüÿcå?ïcƒ'Ø?}(«³¡›?g§ÔU¡á?Wêoõi?™'ÄéPŒ?{Í1ÎBîE4FGL J2321.5-1619?æ?¶ŠÑDÀP¢øa¦
EÀ:2íÈÅ×À<PšíV°@ R""Fô[?û\ãJ½"t?¿']è¾oè?¸½ßÉÿ'ó?ü`q$/Š1@Òú›½
b?ïÆ•Q5}¿æŸCâ­ß¢¿ÙoD]¿ÇM»à~í¿ç€N9Hö꿧Û7TAGNbll3FGL J2321.6-1619NVSS J232137-161935?ïë¥V³
?Të9Ž"§ò?,
¹êV2?!ezdžø_?b™þL«?SáøSJ¿É?ïÅàŠóY?-V6Û©?21²e[É?KV€¦5Ù?{ìŸÉµ&?€0P)-"?îþ§_aa/?'æšä"?e/X5A<?QWY.MÊ?…)-1ì?'-­èÔ!?ï2,}ó?z‹I¿ìî=?S²œ$'-?Dÿƒ;À?˜c$-ùh?zU¶4FGL J2321.7-6438¿î€~®0ÕÀHì° Ä›¦À9µKÀ<p¨O?t@Šû"@ÈqGÐ?­;Ì´Îÿ,?G•๗%?'Õb垼@»¨pL\¿àp¦€Ýµþ¿ÞŒ'àl絿â>=Áç¿á»i˜JA¿å(ǟfb¿» ×»é$ÇAGNbll3FGL J2321.2-6439PMN J2321-6438?ïøÏP_›?Bâ°+š2Ô?çîã!–Š?ã‹ÖÙw?J¥Á®_Å?A懿‡ýü?ïܽ©Ø?zÄ/´@1‰?!¯Ù®Á0?L†ÛÃ÷?q¬F'd:?x·£'"1?ï1ÕOå¥À?€Èu¸HŸS?dµP©	?UXc}øÐ?—.¬6&'?€ǎ¼U?ïúôë¾?8˜+'u½ì>ÿ‹¡ëǦÄ>ó͙ë$?F—/òÉå?8!v÷Æ-4FGL J2321.9+3204?ÙÜ€xá=À;ö<1ßvÀ87[‹ABÀ;‡³äžzª@Øם
gb@Hƒ&Ž? 'FJƒ?¿ò.±fS@ý"$½@Y0Eíõç¿£G>ÞF·¿Ýû†ß؝¿ãJ|àü.º¿ã¬fZ§ìC¿é袠ÿ>¿ëB&¶M.‡AGNfsrq3FGL J2321.9+3204B2 2319+31?ï,´ÿí÷?A=ʉ­×?jÅÃéfþ?f¿4Î6ÓE?—Û…D?‹r,¼g'ã?ï­n"H´q?ƒo[Íŝ?B4"ö¿-?Td6ù?2¹?ƒ®fðÖ?'åt<}ˆ?èüù?–@VÌE›?'QF~Ú?<'™¥Ä?–WÜÈýÆæ?†'â%0?ïÁË+šÚq?lGÿ#^}–?KªìEòm?AÈñÕ]?{¥©ðI‰?j°"î /4FGL J2321.9+2734?å5Ë	À?;Y5ü;OÀ9"¸ÜU
À<4›ök+È@w>ÿ¥@¦pâÁ*Ø?³¤ëÝ3L^?¶Y"€a'@³â…›µÔ@ܰљ4?ïåѶ@™M¿Þ¡NÄ´$Š¿äœ<I	^¿ÜmÍ"ˆ8¿è˜¢ô¿åt¦FPFAGNfsrq3FGL J2321.9+27324C +27.50?úτ$?•À!"š'?u"\$Rò¢?mîë}V?¢·Î}_U?"vå×?íðŠócmt?§å)j†³Ú?€ncÙá?ˆdCîs"?¬ÛÏ0Ò°?¥P×;C¿4?ì )™ë? rDZžÜ	?Ñ~,¾M?€ßë±*­Ÿ?·‡ÝŸN¾?œR?Ž÷næ?얢ÎÇTÊ?•>Ø}áã'?¤ëÚèÏmb?ˆ8òCÎ\?°Ôü]¢ú?Œóø'T±4FGL J2322.1+4440?Œ}ìÀ.·¤ƒ§ À:©È"h¯íÀ<\§D}"@Çs){r@'ä´J?Ë}õ#XÐ?ÉÓQáŸÜ@]týØÞS@þ#ØÍ6)?ín«äõ¸~¿ÙpfÅ[ê7¿æåà/Ò¿ßnwa¶Sd¿ìðZÛî¨À¿ïõ_¯"AGNfsrq3FGL J2321.6+4438B3 2319+444?íz©Ÿœÿ?±#¡·¸¤/?Èg82R?Ž©é\º,?°6ÕËüÔú?­L¼"5??î>R˜Õ^Ë?¥ºmzÊ?}óþ‡'(=?‡Ù}ÙS?¨\V¡·îP?¢Ñ@w¹ÛT?ì+ÀÃ4?ŸÄ°È\³?ŸµúÍ
v?ŒÁXƒvqš?¶¹ V¶Ÿ?—¾ãðÖ7?ëd·ô'V|?—»8B®~?¢ª¬êM?‡?Ïçaú‡?»"éæNƒß?";ŸIAvg4FGL J2322.6-0735¿ëThÌaîÀN¤gbèÑÀ:|©B"	À<Vhiuå_@+ëÞ
ò@bå€!ùO?Ä­Îq?²½)썇h?ìrAÁ@|@|e´å¥a?ïÿT>Eµí¿Ö7@¿åº#ý¶#¾¿äc4^ÁV¿æ6_½Õ¹¿ïÿÀ_V&ÓAGNbcuPMN J2322-0736?ïÞE™# ?jU»3:Im?3sùÝ?.z€Ù$‹C?oLPºÅ?idÄq1?ïË#UrB€?€KpÜäeN?+i†TtÎx?CÈÌzÂl¡?y"	;?i|Cȝw?îÆ(ÐF`R?ˆŠ…ýü?pþ‰~"ˆ?`ä*¬ÃPÛ?¡}¡ËÇiÃ?‡Aí)M?ï"aÌÜIå?qOP-Î?DNvVû?5Ú
Ѧ†H?‰¢¥hè%¦?pùCd°ê"4FGL J2322.7+3436¿çoAL·¤ÙÀ8Ê!§´ÝÀ:ñ
™¶öÀ<T_°i¿·@ 1͒ð] @'5>¦?²Ûù ÜÚ¿¨›ˆ²¼U?öôÖ¡aä÷@BY@ãö¿èŸÁ¦Óê¿ÝçK~-­b¿å§Éþ;YÈ¿Ýu=äçöŸ¿ØºËã˜Á-¿ÔÔúc
AGNbll3FGL J2322.5+3436TXS 2320+343?îæ²éz$?—^È
ÐB?a1
tˆ?Z¦@ë'2? Œ3 Á4?–i(!³?ïQîšçý?'D]ñPàÜ?N^Ó`H?]Å¤âa$?"Ï6
ZÞ?ÅÙ:eѝ?íeô¢°ƒÛ?˜oõg/¯?}ð¶xñŠ?kpw²sw£?²ñO'ìÏÅ?–ÃM·E?íË62øT?'£á5'Æ?sùeגx?cZCç"'?°f¸ÒD,?'Ø`Ø,­4FGL J2322.8-4916¿™Ë˜š@3ÀO´á¼©À9ʾšÚâ9À<
¦{)l
@‹]"•{}?ùÉ¥¶Žj?¹­®#"Y¿?Æj Û'G@ܸŮËZ@ã¸>Jh"¿ïý2%9þ?ïÿ"D¾Â¿Ô¹`¿'F¿Ñbf¼ønf¿åǞ?È¿×pŸ$rüAGNbll3FGL J2322.9-4917SUMSS J232254-491629?ï뒋º…?YjêÀ!­?Vª'É¥Œ?QVO—B•Ä?RÎ?YÁPº?K›ø š>Š?ï¯q£1e´?‡
:öjÕ?BìöàP,ç?[ƒ*–†C?'ôÇÅ¡i?…‡
ì¾?î€lŽÛ
?"Vjïa?‰'³v( ?…½ÖJIÂ?¡£LYr"ñ?Œ#^?ò=?H¯Û?‹uBZ*ëq?k ³àâ?^#Äg™QQ?¥%7?ŠâÔT-s4FGL J2323.5-0317¿æjFDTe)ÀMO½­uÀ7勾åƒ}À;~^ÛWª@¿ÈVÆ`L@HAíá?šo7àü®?¸''	"83@¡e}'%@Éï"µ¿ÑTù²W¿Þ¸ô¾-w²¿ä¡:B-ƒ¿äxfÿš6¿éÏ¡þÂé¿çÞ7u¦AGNfsrq3FGL J2323.5-0315PKS 2320-035?ï`[Gõ?†MÞh"ƒh?SµO
ˆÜ?KùÕ±?'¹JG`"?…Ö€`)æ'?Ƈ|K?iÐub¼Ð?Eׂk²$)?Z|¬c¢÷M?ˆº7eÊÂ?EžèÕ?ï=kkRË?†&òÆ?}Jýœà?y;¬A*Ê?'¿ßŽnw?€£%l–ëh?ïÒ´ðÒ­®?b½€z¶»?@aÁZ"€€?4aéÙj0?t™OkV¹?a­Â	g4FGL J2323.6-0617?¸ÚÚÈâ'?ÀNBàP7PÀ9õ¸Ú§€ãÀ<àŽµ:@‡|"P.—@é=¿Íá?»ðN²º¢?ÇR¿€#@	ÞRù¢í@׵̀?íri^¾Q_¿ÚˆüvÄ¿ä˜Pž¨ø¿èˆ4ýbÁÁ¿ét÷Ãñ[ø¿ïy
]QïAGNfsrqTXS 2321-065?ï]ÍÈhmæ?‡á¹$óÊ?u©¡î#þü?q5»WÂW??·¼î҆Ê?ƒQü¿h?ïМe'ƒb?Žôa"a°?'ôu¶"
ß?F÷
Õõ?vò)‰‰¶X?~-+œ£Å?îE1
4c?"ÐTêy|?'ÊÄAü?.^þ@×?¤c(ü›©`?¬Pã©Ui?ïÎcVÈ¥?b¹:?5=óìø)$?(pŽjC7?w¤ïÌ*Ê?b3y»áOp4FGL J2323.8+4210?瀁ÅùÊÀ1ÍýÞ½À8«€U¾À;"wï$æi@L{)#Ù?ütwéR?¥ÌÁ¶2?±v¡G
Ë@.xžwNì@
Nv/²¿Ù#¸ÁÒó­¿Ò¢Ÿý‹Üm¿àJg,_œ¿Ö(ÑE'пÜzptb¿âÓ¿°.±AGNbll3FGL J2323.9+42111ES 2321+419?₩Ù(Te?œ=+;±˜?>Ê)2¡7!?6Ì:!("?~?ðØ«º?œ8µÕÚÁ?ﯻœµê)?"J…¿?D¤Ò<"Æï?S³'[HjÜ?'ÆË®¼)i?ƒoE]ìÓô?î'cjØ6·?–Õ¾%¿[?wˆ7GžEš?o¤|ȝP?£èÂiˆËà?"‡ª2?îg}‡×"?–ª—&°?lRó4³.?W ¢Ý	?§ÂøJ|;†?=©+ûó<4FGL J2324.7-4041¿¸:Cq|–•ÀPå6&,ºÀ9+þ¤¶-NÀ;¼çºŽÜ§@Øc1R³V?ùùÆ_ËA²?³1`n™€?µ©¸J´¯@å:a$Þ@H€ú?ÁʹÍÇè¿Óf$a´%¿Ý±äíU¿ÓryšÑW¿ÙÊûçA˜¿ÖìsԐAGNbll3FGL J2324.7-40401ES 2322-409?ïאí$qo?j]ß|BM ?7wäbåý?1œjOؙ?rÀ,áÕ?i,LÚ[[?ï׌e'ao?{>ò'a®F?()ü­p?FOí>ÔÍ?syçiܾ?yþ˜§ï?îۏ{Ê?‰;
ÐÞ)?k˜0‰åç?\lݳ¾Nœ? …=…Ÿ?‡°	ÐÍ?îáɽå?‡ŽäÖµÁ?CúՇ2?5
¼ªE'n?¡"†@˒?‡yóRÄKÚ4FGL J2324.7+0801?ßµá聣ÀH†`˜À9'‹©ìÍôÀ<$_iòâá@[(+îz@"­ÿ'+¿?´¾¿iŒá?§k,Á "–?ñY×\rǞ@	Yh&/¿äƍm;¿Þ4ÓpsÛ¿äßd¥Ï2¿Ýx`«¿æ¤"…|+¿æòø°€eìAGNbll3FGL J2324.7+0801PMN J2324+0801?ïÄw|ò?uÞkãmÒ	?D_W&V?<h·ê ?{8]œý?tÛbËX™)?ï¢p£%#<?‹YsïšØN?@˜"yØú?Užƒ8Ÿ•%?†ZUo"€?‰'ëC-Kî?ï4ЈØö?€QaÍ{n?f˜‰cדö?Rv=§Y'z?–'ÝÓ)îÀ?~¦ð"Ó5?ï^Î2´[Í?wiB¥.[0?iÓGµ?V"£d–þ?ô5ï£î?u?ÝF'T^4FGL J2325.2-2010¿ê&z²<—zÀQF¿]xÀ:ú"=_ À<¬˜ÜÛ7Ê@ Q$"‰åG@Ûþ +ïr?¾ôöŒŽÄ)¿´C?šÊœ?ó$5æ€Ó@"†ÔE,?î:ߎñ¿åM¤c!7ˆ¿çti>2пÕMW—Õt¿Ö(`¼ƒS‡¿áæ7¢-¼ÒAGNbcuNVSS J232520-201213?ïX'°Î~?l"èwý6?S~×¢Is?HkvûÚ»?"·Î¯Å{¨?Œ ^BÅ·7?ïŠÌ¿ °?$€…(ø?DàÁø¦'?VÜþϞ©!?Œ9žÄIÆ?ŽÖvIûOf?î 'f"'Ë?'!WÖ¯:#?lJ¥=i?V‹×«´ðZ?¬27üi²ƒ?¨cs3¦ó?î"máÈh4?îҐ¹­?^dCÏt¬<?Tvãœ8æ?¥ÅÿÄý×a?XowÁ4FGL J2325.2+3957?Ðj'7ÛÂÀ3ûªy»­ÁÀ9	Ô¿	•«À;ßʯ¼Î@^(ÿI!?ÿãiÇCöÐ?¨É&O"?½–­@Zöƒ{á@GS&m§ù?ï)KRä©¿½§A"	?D¿âáÝ Y§;¿à—[µ2|¿ä\ËG'	¿ì
³!9AGNbll3FGL J2325.2+3957B3 2322+396?ï´¸'úÌ?|"Ø)í%E?W¹©¡3Þ?V1D¥:Ð?µŠòÚN?y£ìµ¹ï?ô–qÞ?ÏÐçÚr?T]€(',?aDŜJ-?ŠÌ×þƒr?‹(tý]?îrãkØ?•ÈC…ÝÌ?¾nB÷$a?‹&'""? r'.s e?Ž—ËÍÆћ?î«ùv8
¦?…>Kë=V?9-'4÷Ä?mˆF̀Ã? ò7ñçÆ?'/>×ÒrA4FGL J2325.4-4800¿ïVpšFèÀOž¡ß¹8›À9)ÎPZ‹À< }ðƧ@"E³"@ƒV–åŠ3?­RŒâŽS?£T<ò½?õc£Âˆ@2ÃÈí¿Üƒ€Þ6׃¿ánðx£Ì¿âÿ¾øMڿߜè"éŽú¿âár@<I¿ãY¯åC;AGNbll3FGL J2325.4-4758PKS 2322-482?ïå~±E ?^Þ¦ó¥Ý?.ñÞªÈ=W?%¶í%kU ?h'0ÐPÞì?]÷VV?ïË'5?€ðM®]K?/Ìàƒð»]?H‰Ú…ª
?yy×­ßÓ?€Eîœ?ï9ô¬b¬?î®…â¯?dî·Õý?Q}ÉnìyÏ?–#¥Њ½?}ãeŸ¹Éù?Þíƒ?s²½¬ÑÓ?SR­#éE?E‡o'bÌC?†ër»¡B/?ryáéåmÉ4FGL J2325.4-3559¿ÃXN[éÇÀQmƒùdoÀ8ö¬Lú"–À<¯Ù`Y@›©ä'@á%Ie¥?¨dË܌ÞJ?Ç:`Nq@jG¾²í@\¥°ÔÏ¿ÓÝåC;>¿ÛêÆ}'s¿ä€!Î\¿ç1¦k94¿íRCÏb©C¿ïÿ¾ÿ"°AGNfsrq3FGL J2325.3-3557CTS 0490?íùx¤éó?©`+\h?¦56»áø?¥/(šôÒÀ?"f~Ñw?'"ÙG?A£?°x–çr'?v=ÔU&ä…?še
EH?™þ—[?©Ï•Ãò/?éô‹.ÂA?°ìôS4•*?¿	k–oûÅ?¨†ƒÞÖtÚ?±R:øÁò.?£Ü"áå?ïck›™¯à?z˘|íN?rM:šÌäÔ?bùR!l0'?þ{Ì-•W?v•^@X¼ú4FGL J2325.6+1644?åydM	ÀD¹Bá& À:º$?ziSÀ<ƒ»ðÜvŽ@ +Wdë¼ý?þÖ>J¾j3?Ãrµ)B©?«kÿœF·?æRm —d¶@vӉ)‰ç?ïý¢È6¿Éo8&&Z¿àqkè†f·¿âžüå™Lm¿ÁÍ=
!—¿ïþb †ˆEAGNbll3FGL J2325.6+1650NVSS J232538+164641?˜‡Ûë?˜æ#:u?F¡a–1÷A??^:µ;Š?‡*ƒÄ¥å‰?ÒÉ:?>Jõ?ˆU§uøß?3øû¥w?E±ï¾wà?‹0òW¬'?‡è	®–GÖ?î&v›nçê?"w0<À/Y?qšvø?cÁö}D‹?«eG‡'r?'žbât?ï wñFÜÍ?€Cà­Gð?Sì‰Ïf›?IH*^œ<?š²9:3Ò?€ýØïa4FGL J2325.7+1821¿Ëã¸.'ÀCþwÿuÀ:8(y›ÍQÀ<NÌܽ@Т=­	¹@ÃåZbL%?¶(™Ò#¤¿­w?ö:.?õeU	FП@	Cü ÍU?ïçǟ'UR¿äéŸìD¿è´áMK¿ã›ÔÝ<†™¿ëQ©A­?ڔ‰¤Ùé–AGNbcuMG1 J232550+1822?ïBi™öó?'cØ÷¹7?bç[z $?XS°{µç?•Uò‰Ñ݅?¢¹üØÛ?ï[nøý–?"%súl
?FÙwy?Uç(>Aâ¼?"á](¯?9¨Žµ­:?ï«û‹?ƒ·êú²?p…Ü5RD›?i­ØÖJÀ¬?™f3sGýv?¬P՗«(?ïK¨Ô•-?xàÖ¥²?hün¥gô?V;30ñ?"kb?‰mk?výHî<¹*4FGL J2326.2+0113¿ÙÄ"%ÀK'ËûµtÀ:ÄfõŸ<À<"Ýao†¡@ºø"æßÈ@ü¸oG¶?¿˜p_õš2¿wåh£M9©?¹¾|§ñK1@bÁ5"âP?ïÌ;ýÝ¿×ø¾BEtÔ¿ÝÇ-ügš¿ëö>¶4ž?s"Âïö"ê¿ÑÓwá¸íAGNbcuSDSS J232625.63+011208.6?ï³gcçïñ?¦JÔ%¬\?>5Å7‹?V°ÒH&ß·?'5­WÚKe?¥™óŸ;Ì?ïÌjëbo±?¥<mԍ×?'¿zohÛ?DtIyýM?yŽz¼«¹?~"ä"æ=ù?Uê?Šå~'|ê?t(sÑz°?sè¯ås?£´Š<42?ˆÓ;N#?ïÙ¿Æ|¹?^}÷€—¬?«Ðãqäd?EfGÐã?rÝm~ªõ?^ëçOý4FGL J2326.9-0201?Öã,O"<ãÀLàyåŸ+ªÀ:e^ɹòÕÀ<""ÍŸ@Þ~Ðëj@/FÄàoA?¾ŠÀÏ¿¤«@¹ûÜ?äöÞ¸1µ?þ$qÔ®˜"?ïInÞÛ¿å^m=ðüW¿çº•"<¿éøû^°¿Î)F Mgè¿äC¯'9+AGNrdgPKS 2324-02?ìÒ%솅?¯äOX?y~EbTs¿?w?iºð 7?·ÖìE¦:?®‹¿Ÿ–›ê?ï4=©+ o?œGX•ý8?^vú»»p?nsYXŠcŒ?—èÚð6d?™ëŸ'åû?ìGçB5Ð}? >N2¨Ü
?Ž[vþ‹ª?| ³-'s"?¹ÿÚqª§?j¯Ã-x?í&óà?—"5úP?u±÷x²ž?hü!Ȭ8U?µthXܧ?—[ÓÂe
4FGL J2327.3+4717¿±*dcŸ9À*h–š
Ø¡À:·V¥ÿªÀ<~¦ã@N´C%?ý÷})÷JO?͈ܲóݳ?͏¸š:Ô<?ýýI‡2ŽÉ@X;¯X¦?ïãĕƦB¿è¨Ö]š9ý¿Û"oH7Œ¿ß}…fÜ­ë¿ä± VL<ï¿ïýB äfœAGNbcuNVSS J232723+471601?ï7ž?œ'?ˆóbp+,?g6Ÿ©xü=?[ÚÜÃ`3¸?– ØBÝ[±?‡KlÙq?í¸~Jksï?³Ë~†i§?mÝ'u(qÒ?u$–6^+¹?±M$pûó?³SÁd`'?íf=´bŽ8?–t¾-ÒÅ?ˆJ'=*G#?}C1Žå?±ÄÂFE^?'má@t–&?ë1Õþ2†?"ìhX"À?Á¨Y,æ?u²v€§C?Á\£%ì?"¹Vå 4FGL J2327.4+0444?è"
áóƒ#ÀJ"Ðå`BÀ:Øÿ€¾À<f"Xð\@ëâÈÇß@q…Æ}þ?ÃX"ÖĝS¿™."hƒ?ÍêñûÛX+@ùB·Š›?Æ3h7Kñ›¿å.·£oÜ1¿åÀBŠ3ö¿ãdŠž›¿ì4üa'¿ÈK4Ä,ëAGNbcuNVSS J232733+044740?îC¬Js?¢!¯î v?qÃpp"2?cäy·Ú?©«-HM?¡½ÚÉ@Œ?ïÉΊÚM?†'1ÃÁ?6'jÕhèZ?G­L'¤?‡Øùž%Å?†¦ƒ³ ?î`dóG˜l?ŽSÛúT?zˆJµz?lÉÄ7»?¦¨"Cž?‹¨·kxú¡?ïuö2é?q–œ©Ö?Q±¶DzÌ}?@ÍδÀ(‹?&÷Ñö!?pøΆ¢Ð4FGL J2327.5-3259¿ëßƛt)ÀQ½Œ¨À:·pÔ~qöÀ<­æcvÇÝ@ø4O'åJ@3fÿéYË?Ë:Ïç/O?Ȃ;òŸo?ú'(bõ˜ž@¶Œ½¾?ï.Ô>[/|¿ÝzX@ˆÜ2¿çU~¢u¿ée2`=W¿ð?ïÿãåîAGNbcuNVSS J232747-330130?ïÎïð…?s<¼F/2ë?KsêGoí~?EâîK•?uŠtˆsM?qê8&i?ï>Չ°?žC†õ?f6$T+û¼?}Áb"Yß?•^ŠU(j'?™‰&Y?ôV9?Š°¯ÿr.?~I%æÄ!?rç`jhMk?¢žõâsø?†¹N¸=µ/?­"êÇ?v‹õ@ã)û?`ðÈ°DÖÅ?RÕä:œæ‰?Šb¢n´u?uP^‹²ˆ4FGL J2327.5+0939¿ïû{j×åÀGü£a™xÀ8¾®×ï?¾À;§:-ù7@w"ìá•@tõÅêZ|?©4'yì€?ÀV:ߤë²@'bØ<l˜@µÌCŽ¿Ê
2îà¿äõÿ 1#¿éŸ¿™£¿è™cé´d ¿í‹Î2JU¿ðAGNfsrq3FGL J2327.7+0941PKS 2325+093?ïês^ß?fÊý6¿?Rc43¼²¡?aŠ¾Ó¬®?X¶¯…-?X‹eFÐÙ°?ï¥g%Wæ_?ˆ•?§n^?CØ]öÏèª?[¼‡à­è?…h°Ê™ii?†è~q²¼?î¦Ã'¥#­?'%í=X
?…y"a5â?'ÿÁ3? 5eÍ`…?Z'Í{Í?ﰖÊõ.?pïM«²˜§?YÓá½n?M¤¹â,o?€·ý}?n‹Ræc"
4FGL J2328.3-4036¿è?ÌQZnÀQ
-à
qÀ8•t/|ÅMÀ;¤BW"dÌ@—);¸'Ù@©Cäõ?£–œÂ¡ƒQ?²½g4@H/yjO)@ǶãV|?Èd¤Yæü#¿ã²úÉ_Z¿å5¥Õ?¿ä%'(]í¿êÅ
á?¦¿áĆ!—ªVAGNfsrq3FGL J2328.4-4034PKS 2325-408?ïv{›ü&#?"NP‰Î#?X1Í@ä|?Pd¶bœú?Zõ‡NZ¼?ƒã[ü%çê?ïÆ4AéQ?…'fJµ 0?3·æËØWQ?WÐ̤SÁ'?{ªòMѤ?ƒéÒV?îÐxŠI¬ú?sI;ä~â?|–F¨Šø?u´¨,ÐQ?žË]§¢Ó?Œj›Ê¤0?ï¾h}½:?hX»ƒ9õ?F2/ª˜?:IYW·@?~}»Ée?gK«ƒ"ª4FGL J2329.0+0832¿î˜ëme¢áÀHúÁҝÇÀ:X‰ÀßÀ;ú"õëª@	8BÆ¢@¡Ý»1™Ö?Ç/Úx±íx?"%îbYø€?ÆN³×³Z¶@ãçiܹ¿ã6|=鵿êMf»ü¿çµL»šu¿àJæ
²û¿åéázÙºò¿ðAGNfsrqPMN J2329+0834?ï¦ê,q C?ƒ<²P¨?LcÀ–"ýI?Bëˆ
è¤^?"8Ú.Ÿ¬?'õó¸°1k?ïM!_Š@?–O/I¨<?HÍ´ò?˜?V¨€@Ԑ(?•–N,~?•«koÙ8?ìŽè°Ný•?£©¢?…cæd6©?v/R׊ŽÎ?¸ÜX@»Œy?¡ w¼'«?íóLiž¿=?'j½N‹¥Ä?[,›!ŽóŸ?If
E9?¯ñԍ"'?'A¹ÞÓÓ|4FGL J2329.2+3755?ÒÐM\î»À6(ö¾7ޔÀ9œÏýÚÀ<ÂVQEm@ LêÇϸ?þ"]"<?±K£—tP_?Œ´íTy u?܉ݤ`r@"UZ$Ž«?ïÉÁ_[ZD¿â	€,A¿ã&pA±{8¿Ôúv=Éå¿Þ›‹Œ;¿Øp¹[UçAGNbll3FGL J2329.2+3754NVSS J232914+375414?ïE"
¦ÉT?‹ÎvøB÷?U"¸ÉÁä©?K¸ÖÙª?•ûR¾Š·!?Š¹1ë"ôí?W9ø2?†ZO¥˜ ?=^¨ 9)?Më/áNáT?‡óg<@ñ…?…€8ý?í¥ìÒ#p'?—]ØØ;?{tû9Q~E?hÚGÜ8GÌ?±I»Ofß?•bÃI•H}?îÛ3^€?<­Ýü?z]2c´?b¿%>³¯N?ªÖšãÝ«Œ?‹öÝ=4FGL J2329.3-4955?àÝð-ŽsÀO'L Â'ÇÀ6×TûÚ×RÀ;A.jv–_@¾5°;@iÂÝ`?‡­ºÚôƒ?»֑ò†@,úuFÓùè@"ùÃǕ€¿›oðAµÆ»¿àe•P^½%¿äâb`Ght¿åšÅ都¿é°
Ÿ@L¡¿ïHG,{ÄAGNFSRQ3FGL J2329.3-4955PKS 2326-502?ïlÚÉol?†–ÓXÞû?cDwI'¢ ?c+郗e?ø`»Z<O?…§|y?ï3j–(?¡QoðN*å?gx»¬.w?€i«¼˜Ä>?–£–ë%w®? 5Š³ÀÁ?îMR«ñšö?81VÂ?
?ðs,?–X]w+Õ?™Hj'².
?áܪÆ+?ïá×@9?hùó%¬\³?BµÔQ«Ñ?DT¬™Y?i{©ÊÛ[‹?g]›xe04FGL J2329.3-4733¿ëº'´óÃÀPÂÀð À:FM½"4ÞÀ<P!ÀD(N@íb ®ì@ä1æ,c?¿ËÜ!~ã?¥añÆ\Æ?âùåŸ+©Ò@:-1;ŒH?î>rο济¢o¬
¿æ—"[tšÝ¿âh>Õ¿ïÿªÅÝð¿ïü»!©ôAGNfsrq3FGL J2329.9-4734PKS 2326-477?ïò^þ'Ë?RXrÈÒ~B?<ù×߈Ð?2çr´¬±?TÍGƒ?O¬Ž%ÒÖæ?ï´23?…ëHF^±ª?:,l"I‹?Uðrš"¦ç?'"ÒÏÙX¶?" ð8Wô?ï;‰VšÆ?|áö{Z?p"äÜMù‹?hZB	ɂ™?"i›õª¨õ?x
'?©®?ïlj3˹²?wb¥s5?bÝehÀ[¼?R±!ökˆ;?Ùp¾Z?v%ðkò<4FGL J2329.7+6101?ïÖ.²'[Y¿Ò׳ϝÀ9"å'–pÀ;Â`{jÚi@ ÷u½qe?ÿ9  ?½X¡VÒI¹?±½wg?ó·
1A@9úÄ+éh¿äÛQàG}î¿ÜÑT
H¿ä=Ýܽ¿ÔÐß´0¿äÒ÷S‰¿Þ=Á¬ˆ4AGNbcu3FGL J2329.8+6102NVSS J232938+610113?î±îÎB¨?˜£e-Ò¢?O.,¸?F²'{¨ ?¤dZoŸi?˜G«Hw¯¹?ß¡b>''?ϝЎ6c?_.¶'?uxŠ½Ív?àÇɕ¬¿?ϒŒ‡£Ôà?ëˆr³?¥ll7XÁn?"£E¶¶W?q×¼—^¦Â?À•†ØL+?¤‰²¢¿ã?êè³mðuH?¢k +ü3?Ž'H±#™?}ó5½¶»?Âz½½+úS?¢B‰ìœ4FGL J2329.7-2118¿ÔûˆÿdñêÀQ âe+ÔÀ:ÚJcÑaÀ;홭»Ž@Ù"˜€•@¾0O‹Y?ÂÏ
¿¡–¿‹ã­'Ú©H?Èô{§ìÁ@ï¶wö±£?ï²ÌÛæED¿ë棣×e¿Õ§¢Æ¾ì¿éÍÛU%ÌB¿âQ7@¿ïù˜¨)AGNrdgPKS 2327-215?îfpç~C?¦Q"p‰·?yf©Dèm9?tÔ	¬]¦T?¬\ÃÈë;?¥lühÄé?ï=">»+l?™h,S¡†?[?
	lď?jÒɺÄE®?–™§XÆC?—,ðúÌI?é=<ƒµžÎ?¬cS@H?¡4‹""Ê?È;­úqý?ƽë|Ô?¨…eý_Т?ë­u¹Lí?Ÿ¨€Qw@Ã?{kï=Ûù‹?n"Á1*'?ÀnÉ¡Ëì}?Ÿ8²Uòƒ˜4FGL J2330.2+7759?çu%'µ@X@/œŸ"…]¢À: ÝU±}À<]pŒZö@ý÷ºa:X@⿐¤(?½¦´4P?¾wðýX°Æ@@Äe?@
~åkT6ä¿ãïa·ªü˜¿æE¿ý±q¿ä•[Fw´¿ã‹B¸â¿è‰ýÅ=6¿ïý«Ç™‡%AGNbcuWN B2329.2+7743?ï¼Q·£–˜?u§@ {2Ã?b‡ÀVb"ñ?^¿Ã©IQ±?x"Dih?r¤è7ûŸ?ïšóE'ó?ˆ²²G]ùí?K	¦U¯X?\Ìõ+Ôä?‡'"5ñä}?‡9 C®ù?ïŒòÞÍh?¨X6ôH+?r%F‰¸ïô?h|²Y‹P?˜e¸ø?~ۻړ?ï`ÊÔÀŸ+?w4oÔÚ®?pZu÷–#?Z`<vå¤? ÔVjH?u®Ó"uñæ4FGL J2330.3-2332¿ÏQ¥ö/'áÀQÖ"t¼jÀ;t‡'YYÀ<¦ÞãOÆ@gÄW]_@p Ç`?Ò»ûS?¾P[!¹¹?îրÀ.Ù²@d.'Ü¿ïõúÐ7»?î;¼(ßó¿ç"€$þg¿Û#ð_£ÿy¿âý²}–-Ô¿ïÿ?…¦óAGNbcu2MASS J23301617-2336413?ïÕÀt^ê?i1Æ6<??Þæޛoc?7¹…)µº3?s!׃fÔT?hJ^QKF?P¬r?‹&\À¬å8?DsÅ4óÆH?U~à]'ß?‰–o¦¦Ô?‰®Vâæ«?î\µsD"•?‹좟¢?u*Ӈ?É?c°SU>ˆô?§NZνŽ?ˆÙ–ºž½C?îã]º!ö?":'!'?hèvtwÒ¶?`g²Áë? ;œö¦³s?ƒŠùß4FGL J2330.3-2948?çbõ´ˆÄpÀQÿÐR"JËÀ;Ñx-8GÀ<Áû
Qø@`ŒŠ¸Ö@sgÁLf?»Ío4[\¿·–Õ™úèi?ú#=ó?è›$T"Lç?ïr-^ÝÛé¿â0¶¶àÒ=¿ä/?› '¿Ú©A­Iz¿Ûh¯a,Ü¿å&ÓßÅpAGNbllLEDA 3230048?ïbS<¡?°Ïےˆöf?_ù4<—¼è?`™O@÷Þ?'¶¶p?°Õh¢á›?îBZÕÃì?°ßýtØs?ˆ•G^?šôï̘É?¥µÝù¼?©|F•ÆÅ?í·òðRz?"13T'.?~Ôý¸å?y˜ôçƒ?°Z Ž«€¡?'ʛföB?é2ÔP«m?­ÔÛ<ßí!?¤k»Ú[?˜w‡Q|cˆ?Æ¿ü\÷?¬v=|n°^4FGL J2330.5+1102?ÖÝi	%eÀG‰c4'¾ŒÀ9úŸg8ô=À<¯#nš@ZV'©è@õNÂR ?Ç<5»MÉb?Ñ{Pw@ //˜t@
V¡¢Q¤¿Ô	 ØÅ¿çæáËâl¿ç\Á¡ö_¿îWšPx¾X¿ïÿÝÀåãÊ¿ïÿÿ)@k*AGNfsrq3FGL J2330.5+11044C +10.73?ïñkțJS?XÏÀ‡Çj(??ž|¡Ëüv?9'ìh'?U@Ï ø[0?U@Ú¿É	?î|%‡j˜?§ÃnÄ;‹Ì?v6¨ÊÌ?"~üðdz?¥yàRpû?¤ûÐ ‡û?ì·40BµÑ?  ñ Å?™|¶Kÿs»?‰¶òÓ?³ç0êêt?™ó•i'å?î_E·¥"Š?Ž4ó
T÷?'ÔGëP?C?p %2T?¥V'ŠÒ§ˆ?‹¾zñçÝr4FGL J2330.6-3726?·G¶£WÂæÀQ‡ ù	kºÀ:MµåçPÀ<=æë\@'"Æç@#¥™'¥?³çW'Žž¿±ÑÅÁ&¿?üûÅÃď@6càÐ÷?ïNË	~.¿ç	ÃÞ;µ
¿æu^¡ví¿åw¥[Zš¿ÙUÛ}¿ž¿çŠÄê€;ûAGNbll3FGL J2330.4-3726PKS 2327-376?íÿK¸ÇM?§€om†¡í?u*÷Ëá.š?jdbΧ>?­h¬J÷e_?§	69¯Ô?ïfF;ÊÓA?•yOˆ‹vj?T^)ZçÞi?hìIªõà?'ñUð÷?"½£wßk'?í=ÌÇÀQ5?›5&Qy¯?†Ó#à?uä$^BÕ?³Q_a­'Ï?˜|
·<'}?ï%–Ìaõ?€6…—‹J?r+ÄÖb™?dý²æû£?–Ô›ðÛì?}ï–Ï/‰4FGL J2331.0-2147?åf#µç­úÀQ¾5'Ì÷À90b°Ï@À;ª"Xð\@BÏæ\ÀË@v´âË;Ó?°y5 W?À³³á™b'@c™,ŒP@¹@ÓÚ³¿Û9Î¿Öï=Û,áà¿çñZëÞàÌ¿åW¢žzÿÑ¿ìÛªëÑtÒ¿ïÿyB=KAGNfsrq3FGL J2330.8-2144PMN J2331-2148?ïÓÈEòÍ?hlh½"Íå?_Œàԋ5š?Vyªž¡Ëc?m1ÇOǘ•?c¬EÀÌ4?ïÌuÔm¿†?1Ӆÿp?0úˆ¤ÅØ?KS÷•
ÊO?xµmHåð­?€Iل"?ít½¼t?s˜Ñ$?›§Û{\?'ÄX0{¾,?«)ÐQRÐ?•i¿mÌ`?ïÖ9‰•w?t[§Nòö?X Z°?LÅÛÝzf?Œ†ýL?sPäkŸµ4FGL J2331.1-1653?ÝØËG*zÂÀQ3y¦µÀ:êDrØ
À<G¥rë¯ç@¨+i:V=@
˅¤ð?ÔØ[
è'N?³
f
uú®?á"	¶@të¢%p¿ãT°',㎿ºcß½.8¿è7=^ZS^¿ìë»%_5¿ïþ®[È}³?ëUI°ÎjAGNbcuPKS 2328-172?ï¤Ü²ãQ‰?´ÛÂër7c?2v0'Q?FŽ‡y#1ý?†8/•§
3?´Ú…PþÁ?ïu1WP?"ˆqÞP9ù?Rãwÿîw?j‹µóñ?+Ÿç?'J2°t+?îËãQ*?"'ÿ	=?€‰à>ÐFd?x@òΩb?©ô{2ÛÂ?'3Ûüì?áê›?uJŒ8ãqª?Ao<{S	?7,îNܕ…?ŠE½Ê§¹?uÇ_Ê@4FGL J2331.3-1558¿ïº™^`]ŽÀQᛐëÀ:¶ÇǪNÀ<TtûTŸ•@¥¶Ê,@ÐE AY?Ð6̤?®ÆßԈÐ?ÝW¸"Æ©r@
³‰‹"ƒ¿ÊöZlˆ¿ëyJ]¿ßUûļ2¿ê†^¾Ò8G¿á(&à>™™¿ïöÕ´ÒÛAGNfsrq2FGL J2331.8-1607PKS 2329-16?ïЬ‹W—?tx8¨ˆ?0÷Ø%^iP?'èà¥W¦?vš<Ñސß?t"*Ï$¨?ï¦N%.'3?Œ2PoðÛ?B±g;f¬±?\ûL,G¤e?…A`@¥¶?‰åÐl¿°?î àÉ»ðp?‹*}{Qµé?sä?­á?mŽ¹¡Ûš ?£öÜK<×?ˆ©x¿ëì?ïxÏØú/?tÈš[«?1Û9þˆä?'Œxï—?µyæš?t²ˆþޗW4FGL J2331.5-0258?ëx®+eÎ*ÀM™ìòù‡À;m/®CuÀ<'Ô{ø@ §6…º?ú¹Ð¦v ï?Ó¿²ÝãJ"?Ш $ã1?ü@j‰
Ö@kù«R(Â?ïò6H'iI¿èßvBQ‰5¿Ì/¥ßøù|¿Ù(ë܇ç¿Ðki$Ü®A¿ïÿÿ" 5•AGNbcuGALEXASC J233112.94-030129.9?ïÄxAüî]?x'Å_§'À?Bl`鋒?@' ÅS͟?{€quk ?w•àI0s?ïšNóê?‰à"mK?@îÚ&XÜ¢?SD{Û%_?ˆ]ŒàÓ÷"?ˆ§N¶/+í?í›ð‡e†_?˜Í›ˆGç[?vÊÿŽ`õ?qÅ׳ÙøÜ?±³ÚDÚæú?˜3÷¹??î"d­>ƒ?Œ
îZ>?B•Ò™¨¦¸?;k£òÒ|C?¦]á¸õ'?‹öêá3µ4FGL J2332.1-4118?ÕºîmÜQÀQÎþÖ4UÀ:ÇÑ;ÇVkÀ<{èxú½¡@ûs'
@݇»¢?γ$Z'hÐ?؆~ŸBP@¬}Cø}U@"E¬/ô¿îß´tç?îa{zÊ¡y¿Ú@H%©ˆ¿éeDþ6Ò$¿ïôZ 4"[?ï­¹¬^˜<AGNfsrqPKS 2329-415?î/;ÅÇ8!?£6??<?ƒÙÂǗ>?ƒ(4ú»˜?¨+Í2ژ?¡‰ó"èF?ìéÉ;ÎP?¸ùޅ±û?ô©àc†?ªÛ,^Ÿ×Ð?±4‹àqt©?²B>ø±y?çù³Ò‹êÀ?¬/¥çDÈÌ?¸×욟?•76[­…?í©?ƒr?¥LÚ¹4?êº+hóÛ?§Å¹¼
Os?¦ÏzjÊQB?—x Yªx1?¾Æç'ûþl?£¾á(ã}–4FGL J2333.4-0133¿Ïz~á²bÀM)¬îàóËÀ:¨Ó¶ËوÀ<	Äf̽³@¢PE½¤f@[›Äí{?Ð<}>šœ?ÊuqǬ?ú]­	¸æf@dõu|Y¿ïh;ibš?ée·ýä¿åž¸‡›jT¿ëŽäŸQi¿ã=ÓLKˆ¿ïÅ¡—ûAGNfsrqPKS B2330-017?îmœº/ŠÞ?¦únØñá1?zâRõ?}îuK?¥Éà¼<ùº?¥n…ñN¦?ïða¡Tw?¢æ?'0A?f¶{¤d?vµåŒ¶­#?™ë0\`äi? µn
/(?ì¼ÿsÒA? ÑvâŠu?'¯Ï•˜'"?ƒ$æc(&±?µ¬ÞûMR?œ»ì˜6Ý?í
ÏäEü·?˜+õ̓–ž?yøzÐёÇ?n
Øó?¶	ù0Ã+?˜$H~{ë4FGL J2334.2+0736¿æÀ!¿S£§ÀIGFýëRÊÀ::DŸlAÀ<3ßTŽÍŽ@}³Ö†´å@ŒÏ¡"c?»ñ~‡ðNÝ?°`u¶uY?í¹Å‰¬Ü@uu‹u•?ïÿyYˆ¿Ùjh~™Ž¿äƒÆÞ÷Ö¿ê${àK.Ò¿å'XýÈ[¿ïÿúŒ"¸'AGNfsrq3FGL J2334.1+0732TXS 2331+073?ïõ–ɤ[6?R¼ýÃXË?˜só¦?"•ðê–k¡?S s0
W'?Q1¸E[&5?ï¾²¿dg5?'–ñÁ)T?-­Ío)*Ý?CC"mŽ>?¹1âS™?'ºÆÅhË?îÜÛS!ÇF?…ŽªœQgà?v:½³"oì?kè ©?žÕæ.áû?ƒ.¬÷ ×o?ï¸UÃU	û?g2©0ªL?GzN掕å?85VÒuۍ?€rê<T˜?fW‹‰h•©4FGL J2334.8+1432¿åáاmåÀF1(bõ˜žÀ9|G6v¾À;ïXÒÿìµ@XjGFˆ?þl»o?®Ï†C.0ž?¶'Ëïت@æ¥×Û@;FY€¤Ö¿ÀFdé8¾8¿Äa¦ù~†™¿áéàÙÊQ¿Ü÷jU¥#¿Þ¦YÛéuO¿î$…á*ý°AGNbll3FGL J2334.8+1432NVSS J233453+143214?ïð•v}L?QzðÑJ?*5ô%˜ž—? öÞ¤?[ŽUTRTõ?P«ëU€ý?ïÀ½6PzŸ?5C
üÏ?5
ސöL_?Z	äÂß?~P†î³K3?qLPßô?ï
!ˆqnõ?ƒ:Ž¦÷é?rÐì·Û¸6?oÍÄ,9-É?š"ÃÛ3?~»Ü©÷þ·?ï·QsùŽ?fÏcOª›'?/Û(z¬Ð?"§ëG
M?¬OAé"?f{Ø3ÞÜ4FGL J2334.9-2346¿Ù'j;=ÀRÚøßzNÀ:$Ú¯ä^ºÀ<aJ©q}ò@ÎRв_Ž@ܹ>z?»)9à '›?ŸÐb¿¤Œ?à"´/Gh@®òÇ2Y?ᅴ÷Aë]¿è%5y^¯¿æª>,‹y¿äùw_Ýá¿ìxá=G3¿ÏüƒHÊI:AGNagn3FGL J2335.6-2342PKS 2331-240?îþý§·×?"ߪqäš?mœK<µªx?aÈ¡l?œlÒ£rO¹?'ì-çý@€?o]_3?Ð–¤°ie?I›Œ¼ÈYA?`àåTóI÷?Œ:k\Û­f?´¤¸î֐?ï	\'ÜN?'°Ënm"?pfa!`¦|?bœ"‡¨l¡?šºçr¬LÖ?€¾à³ç½ã?ïv1A"?slÃjWyh?frÅËSñ?T ,2¸‹?ŒÞi¦?q¡®Ò«c)4FGL J2335.4-0128¿ìÎ셵ó(ÀME>>)0{À:\+ŒuĨÀ;öȋ­@]ú͑ë@	Þu?Ěº@ƒ'è?ÓÖX¼¯ž>@
tBâӟO@´r€s®?âUT€_὿ä‡"Ô@^•¿å°¤xí¿éëâ§)¥¿çç™!#¼¿ïõQ@9AGNfsrq3FGL J2335.1-0133PKS 2332-017?îJ‹Ÿ•î?°áËË{?'Âúr=ð?"/¾%k?¢Pä'm''?ª>Á|(à?íòé4¦G¸?³;É#y_?Ž¿Çº?1C?£j'[¤?©!zǸ<?«à·Ô+ÜÊ?é'öU1í?©rÈ£›à?°^ï?¸%?—°¾Ñ7Ë?Áį( :?¥
9+;Ôb?éß/菉•?¦ü^&…Ù¡?PTe_Ø?€þéÝdM®?Ǝ;kÜ%?¦œ0páw4FGL J2336.5-7622?è5jôQRÀCõ¦ZÀ:d"j]kìÀ<‡ó×ӑ@Ä%4ÂÕR@«ÈÛ¦"d?¼¸€uÂ`?"þcGÍõ?Ôà´`Dc\@¥¹z׿è7ŸS—Ø¿Ï"na‡"n¿â2/ýô¿å"~Z#¿ãÞó`4s$¿å"à\÷RAGNbll3FGL J2336.5-7620PMN J2336-7620?ïÄFºO:?rÀ;ôߟ?LZ¸62Ø?B©ìOÅn?zQKÕ</?q£b/ïQõ?ﶎ;¢=?'*@u™)?'ZÔó"†?=2Qâ\â?ÿÈËV¡?ÏÖ=Ð-?ï'"Šq?ƒ\ì"òL.?o(»s/?a'¡«ûv??›+(múqI?md£?ïµÄ0èãK?h¨{Põ‰ó?PyágÒVW?>47sMHã?€·˜Ìâ
?hM½Ñ½%4FGL J2336.6+2356?ÖÑ7{ºÀAê]yЦÀ:'ã8IªÀ<}\ã/å¡@sòvŽ+@‹4*©ø?À¬Ëxº?°Ö‡X¤\?ñ´)¸`.>@'#uP5¿ïø
ñâ?ïÿ*'Š‰[¿å3¢Câ-¿â•"z›¨¿×Ⴜ]hç¿é؃""^ŸAGNbcu3FGL J2336.5+2356B2 2334+23?ïqIJ:?"®,@œ?X
¾´S?O"øn%]?Kzëw½H?"''ÝE?ïTXÀ­;?'¸å›Ä>‰?L7~gGâx?]5uMªC?""A"°"?'²¥)zL´?íþ"úË1ý?"QDþ¨?|_öHçüH?k6'sŽ$?¬Š±Š/à»?Ž|™Õ¤q?îÓu_WE³?'ªÑïtä?|8,՘6?okC²"¥?žƒHß±F±?ŽÂ®Ë
c4FGL J2336.6-4115?ïñRY­àÀQHÙŽuyÀ9—ÇÜ£¦À<$«:«Í@Ã×öv"\@»tÝøn;?±dáVÀ{?½Y(ÿíOh@	Sü¡¦®U@zßøx¢¿µ+Pæ¢`è¿ÝA3¼pQ¿åO°!Etÿ¿æГ€ÐÊÞ¿åWõT«S¿åOß;AGNfsrq3FGL J2336.5-4116PKS 2333-415?ïèñ5}_?ZβRS"Ú?3K'
·¸³?*ÜÛRi¬?d¥f˧¦?Y\ƒ¨ic;?ïÛ^lø?yfÒ0øa?%ʓ)6?C<¢Oÿ
?qÍ|1›ºÄ?xc"üžë?ïQë?…×:ƒT¦ï?u+(Á@3?qޓJV4Ë?™+­¼½?'¢×&?ïä2"®h?T^¢tšÁE?0"d&*?"z2ÃQµ?iʽZÅ,?S—ÚÒ4FGL J2336.9-5859?êÈm(f?iÀKÐ<³åuÀ;VÅÓ´G›À<Á ªšrÝ@/ª›õiy@¸™aeu¦?ÜÚ]-W§?Í·Ÿ©~+?çx˜˜Ú@X…ïBÃt¿ïª'ñ¶'!?îa«IQ¿å¡­>¼ÿ$¿ä¶+ÀÎð¿ïÿìêy…þ?î9æ@;YrAGNbcuPMN J2337-5901?卑ÀIZ9?5Í9Vª÷?Z~ƒçs9µ?cÞ]ó=Ç?''¿p»
B?‹œM;?ï†^æ3^?ïäÒ7<Ñ?KÓ±ÄQÄ?b'ÀsWk?Œ«=ê1cN?ƒ™ß£ˆ%?ì'.–t?Ÿ­ÃUø?÷;
#?ŽÖÝAM?´pÁ	L'?—Ü–QC^?ïÄÝ»¨ÔV?j¬æ{«%Ô?=ÏâN|&?B,•ý7¾™?{´$
0í«?i©Å4FGL J2338.0-0230¿ë‡öÖ-ÊÀMàÐÜüŹÀ9/{T44»À<
ª}í@tÐ%Ǻ¿@¸t »ÌÊ?¬¾lô-u?«ж'L?üu`4=þ@yFCcA¿×Â;cÙCS¿ã6M½øô¿æTŒê^®¿çç¾Àš¿íäŠÄÀ§?ÆP²ŠMÈAGNfsrq3FGL J2338.1-0229PKS 2335-027?ïÆÙPªe¤?sñ³k¶1?E#G=?>l²IÃ?yîæìeç?sET骒r?ïÑ挋
h?~¼®FóïÐ?-4±ê3žø?Köo<½?v#+'¯¬?|ÙËaaÈ?ï$™z*€?r͕R·?pÖ~§?cé3Ùb`?—7,¦ÚÌÚ?{¤9ÝL«S?ïãMå¼D?X‡æZï	??5…ªÔô?3ä%.ìÊ¿?hËiŽ"=?Vp‡wó4FGL J2338.1+0325¿Þqn¢u
nÀKX³!ž¶À:ÁêÃê¦À<AF¹!õ@…F/9T@óMAÒ2g?ËmÖݜӶ?Æ	ÃbÀ¿x?ûI·ôÎs–@6+™Þ¿íÀ.ž£ï‰?îjA¢a¿8¿çöLÃ'1¿å{î|Iý¿á©Šrµ)B¿ïÿýç!éAGNagnPKS 2335+03?ïAËÿž9ô?$ë⃓Ÿ?{_ÕÌ<(?wyëÞÚS?î¸ÖŲ–?‹~¶sÀ?î¸Èe?£–("ŒjŠ?lw1ÎÇ|?tò ôá-_?¢· bºæ?¡æ‡›ùñß?ìÒµ9£?›uXV1h?'VÜ!¾T±?8ÌìÊë?µŸ*tð?—_(Þbñ?ì¶äNÚs©?–ñՎÅ?ˆ¢ðˆG?yj-µþt.?·4‹ËYÖ?–¾adl{4FGL J2338.9+2124?èÍ5QÀC2¹^Zÿ*À:»ö»³ À<UCh4œÀ@_FrÖ@(è6ú?´r4ûµB—¿‹v±ÚzÉ?Ø&IaÉ@(Çí?)?ïÿ¢âîwA¿à"-F<$¿än$Öyù¿ÞpDAùJ¿ÙK"\Ðg¿Ýô½ÑâAGNbll3FGL J2339.0+2122RX J2338.8+2124?ï4Kú?Š¿æ™t/?GØnrm³?A)!xÜÊ?ŠufTš Ù?Š} "ê?ï­l¶e]?'›[ޚ¬?1C¢ìñçÝ?DÞ†&U?"µOW™ô?'C,uòl?î£Å!í?@Ȓ?iˆj™­	Y?\à–'õ?¤+'7"æh?Ž½¹¥/?ïXÅúuö»?u»ªBӟ]?\	@â+ËÎ?JqÙËxg?"&¬£k£?t楏V4FGL J2339.2-7403¿²¢÷QGÕ³ÀE7~ŽÒÀ:—âà4‰À<yyRژ@X*"~&Ì?þ¤(hÔÕ°?¶äø½–xþ?¦Õç}¨!r?ð˜í×ßO†@o[¸7"l?ïé`ŒÝŸ¿âÕÛN¿àÜ<ÁÒGá¿ÛOBŒf¿ãy«ó8qa¿×À
6Ih)AGNbll3FGL J2338.7-74011RXS J233919.8-740439?ïÄåÓqP?l㈏xu?@ҔÀS?J?2üó²®Xþ?{rïMWQ?k{Ù©=pê?ï"ç}ûÏF?‡è.¼YšZ?6Þ<†î=5?Fb7øTñG?ŠO.œÔ¼U?‡OŽ51a?ï%W¶=?€(›Ùã""?dŠ¬I31¦?SÈ Ú?6?š	ÿ€²8?~F,΅º*?ï<á6U¡à?wJCD!B©?h&:°yª?QÓ4¢*?•_ßGôÚ?v1ãÂ&· 4FGL J2339.3-2656¿ØÞ9õLÑHÀR}|o½'=À;oˆ"xÐÌÀ<Évú2`¥@í°°ŒzL@Wª¹|ð?Ïå5¤Q®s?Œ°'¿7á?¿ø¢~¶_@»©äÀ^?ïª9ú͑¿çôÉ_¿åÕ¾]ž@È¿Õß/»Y‡Ü¿äÉï•N±¿ïéõ!T¹kAGNbcuNVSS J233917-265638?ïÃ69©¤?xðIâTJs?8º¹ÈBJW?0Ø×fzZˆ?|Ù7Õ§	à?x\[ å0?ïµlÊ5W?…ªÉ<&µ¸?6aõ½äã?N^Á'ÊàÔ?'›ÝÄ»?"®˜šÙ?îµ!÷ðéa?‰©àÒ8@…?gW%U$®›?\Öޕ¢?£8n+Ÿú?ˆ¶€N…?ï¸kyVF?g€.êd¢
?1'4ã<
?%Ê!ÁPË?YHÇ_[?gJ7Uj4FGL J2339.6+0242¿Ü—gÔêAlÀKÀ"`ÑÀ:$رÝ]>À<+ÉMì@¡ÑÖvï¡@GPܑeî?ÃMK7`êQ?É¿?#€c@ù«ó8qa@
£E±,?ïܨAÓ	'¿å~Âþ—Ë
¿ç¡]]SBG¿èÉv7]d¿ïø[#*¿ïü'«@‹AGNbcu3FGL J2338.7+0251CRATES J233930+024420?ïÝó>E* ?ˆ£r.o…å?aG'qÔ6Q?ˆUhêçpà?`Å?Iª|?\Cãe¨˜?î]1DBé?§®|jâžç?~¥c{»"C?"ªLÝÎÝ?¦X?Pd_?¤¶Ê†<À?îŒ"Q¼ç?'~þ¤ò?†㳚¥?{ìQ+Dï?¡¸¢½ˆ9?‹6Í`Ä?ívgQ©{?"ݬؔÎô?–Єâ?ÆR|W'¥?²+¥*»ž?'7Rq•ŒÒ4FGL J2340.5+3854?Ы²d°sÀ5ëVûW÷À:á½ñg·À<…üÉêš=@ Ih«»M?þó•:a%?Èîºu\N?©PÃß4к?äfg=%û<@1" k³?êÚÛé*Ñ¿ÇÀ[zO&"¿é´ò?øé`¿Ô°– ÀÕH¿Ï^c¸Œ¿êg%©ôçAGNbcu3FGL J2340.7+3847GALEXASC J234042.83+385510.7?î"z-ö?¢écW…áŸ?ZhÅŒW…?P¸Ïg·ö?­JàX½ð?¢«¹'3, ?ïc‹BÎô?j¢éo?D1`Ì蹨?Sx®·¤?'íŸº9Ë?ŽäÑ\/?ížK#´iS?"-`¢ —?t¶­ÿ?cݐ5íVë?±Ì+w|ÃÓ?'E¶"ü…?î
1r©RÐ?‹ª€&ÁÓw?k'×¼£ÜÜ?^¡ôÈd~'?­£»Y •;?‹S~¨£té4FGL J2340.8+8015?좂^>¤«@1Ðx·¡Â]À8»ZôB\œÀ;œ—ü
§ú@ Øf3Í?ýmlš]
ø?¦/ºîí‰?·ø«wènê@Qš&‡S@uþÕ®Ë?ï¿t¿Å}M¿â¯LåÄ¿ÜÂ~_o׿ԈB#þÀ¿â\ʵ›X¿ÞR+[xv´AGNbll3FGL J2340.7+80161RXS J234051.4+801513?í7ˆ}ç&?ªˆOz8–ˆ?‡OZ?'I]LBä?³aÚ-d?¨Î€£q¤?è`¥Å¥¯?Ç`Ãù§_?¼A¾®jÒä?Á »CÔ«?À^²³ÿÓ?»]º
˜éþ?èV׏«,µ?¯ì‹¤›	t?£» /?'ÕS轔þ?ÉãrÙRŠ?¬ø¨©ò.h?âN	þ?ª7cEô!?Á}rˆ™|E?¢t-Hª´2?Ó8ª¡'á?¨i 0áÐ4FGL J2341.8-2917¿ØžeáØ£ÀR¡quŽ!–À:öä/À<±páêkC@~¯—ݬÄ@ۀ©Þ‹;?Ìs‹èÖî?Àx)Çόñ?ñàV·œ¹à?ü¢òÙPé§?î³àֆ¿Ó¬p¡RË¿ágž	jâÍ¿âBl¡"ãø¿ïÿF!!Ä?ïù‹a~ÖAGNrdgPKS 2338-295?ï|ñœ9?ƒlÿ"I?a[217`¾?].E"óæè?ŒlìªYr?'ŽðÒö£?îà"€ýb¤?¡€É—™À?p©6þ¬¢á?{xYM	ˆ?ŸÃ" ¨'±?ŸÑI_
Û?íF¹øx?–÷¯Ið"?•ÚÁšÒò?ˆªyï
'–?°Sô•R©?ëŒÕçÄ?íjë¼f?—KU
<ý?†^ìñ›£x?y™8n^:?±Üā[?•],õ÷I4FGL J2343.6+3438?ê/'¼³O"À:.o`àëhÀ:+'›O|À<>9E›ëƒ@ á{´×7µ?û=uâlv?º…™\‡ëF?°ZKÐãݵ?ö T3]û^@Lï‹h©b¿ïԍöÎ(?ê`=X¿ÂÝÚ%ÐÊ¿Öe
{"Ý¿ÞÝh»Ö/w¿ÅWÙc¯AGNbll3FGL J2343.7+34371RXS J234332.5+343957?ïåq¬áƒa?b¿è3!	?1Â
÷].?."÷ª¢?hV|½³ý?aØ;5HG?ïÈ™Ëè?õ&
qÍâ?)ŒKt5?BÍÊì¡Aò?{,ˆ¾d?
'í.OÃ?îéæ¹u;?…¥©ðë?g
eˆÄÝ?]Ìôz3kð?Ÿá÷Î_ý?"ŠÁí?ï@ÅÕï?w×ØO×lQ?YûŠû$q¿?G…;n‰Ú?–G£U×Z?w;a4FGL J2343.7-5624?î'ÜqÀM(6CˆëÌÀ:Íã˜Á,†À< †TBw@Â>%Õ|Ÿ@ç<º›qá?ÀÊ¶Ú ¿–rŸj`h?Ôì¾Ü-"@Uf¤S1?¼æ+ÿžlx¿ç¶Â3얗¿éÌVè'¿Ô¼Ì¤ˆàå¿í=Û,áàZ¿ãYyMÉ·oAGNbcuPKS 2340-567?ïâ'S[u?hÖµòt¸z?FO³+µü?=ñü¶a"?gÚ¿Ù÷GÐ?gj|˖0?ïÖـ
?zI¿¡;ðæ?"ñ8S"?:CVkÂà¼?tˆo;`b?y~VjÞK?ïCj[öc¬?{G_Üê?g¥±Í_&?^ùH6øt£?"þ`yޑ?x…´³õH?ïäËÕ/>?Uü0žvÀ?<H§'QˆW?1)ŸáóÃ?hn:†'=?SÀbÉýu4FGL J2343.9+0546?ïzéîEÃYÀJ¢pCßÀ:ª¶P‰…OÀ<iDo›™N@…Ã÷¼º@%`â˜ç?ē['÷
é?Ò­Ûzº†N@	»ž ç×@J¨;rò¼¿ëoyȸ?ѼB¦m½s¿ã
,kü¿Øò.Ü"¿éΕßе¿ïÿëÞ
òAGNbcu3FGL J2344.4+05491RXS J234354.4+054713?î1ÝݒíI?£ˆáƹ:? ù$£ß?œЙ	šø?—Ñûä)î?ÝzŸ¿k?í'ŸˆšM?³š<Ádk?'ס«H?›;U|B–æ?²
wD]…?°DÁ€Ás ?éˆGEÄ;?©Õ»01Œà?¶,¡ýÿ"ÿ? Þ͐N?½'#ÓßÁ&? 8B¸o«?êÈrƒ*/?¢1T37_?¤÷pK¢?'¹Å|i§î?¿DDFXÝu?¾ëÓÉ3¼4FGL J2345.2-1555¿î˜æ
¶g[ÀQ¿j@»À7!–5dfÀ:þO'åJr@Þ_ùÎj@E}àÖo
?'àQ—ì}?ºW±þÑgø@&§lH'¶þ@ª#
¡S¿Ç¼€xá¿Ùòì;}·¿â_Ï=ÀTï¿â?êÁf½¿çø@îݘͿ糝쏋AGNFSRQ3FGL J2345.2-1554PMN J2345-1555?ï|Æ)Eõ?'Oƒ¹Xϯ?L܉SsR?KulF^eU?­%·Mõ?ÚëR‡?ï9ïÀUHz?§_eÐhÛ?c°çÑÂã(?ƒbÔ{ÍPæ?–Kêû"^?¤ÿ±!?í¼'õË?¡¬"1zN?"ãH±´ ?'yÓ8AVy?©Æ,Ud«m?›-Ž ‹ŽÅ?ïRmŸUS"?Œ*#Í©€…?QaþVÚ2?Qˆ"ü‡Ï?"œ,/çìT?‹Rû$5gÇ4FGL J2346.7+0705¿ÇÍ´Ô2œµÀJ.XOLnnÀ9,¨hiuåÀ;Ð֟´eÎ@ 51¯=?ýŽ Ç‹Dl?­-=¿—ôÃ?–oBᄝg?ìHÆxõ@íÈs÷žˆ¿ïÿíUÙPi?ïþÝöÀ¼¿âðûµîcö¿Ñ	ç_u0"¿ã£—I]A$¿¾_ðÀòÎêAGNbll3FGL J2346.7+0705TXS 2344+068?ïÅLŸ4í?|a­Í½×?@-˜Šã?DÓ	qæ"Õ?{Sýcj¬d?zãa}¨u?ï›qj›ÿq?Xai"5­?EдÓ0Â?[ÞëݾFÉ?‡Æ¥=²ð³?
|ƒ(J?í¬ð¸îÐ?žºáráÈT?'¼v¬uÔ?wHEöJö?´³	¤©çj?›ûþ>H†s?îpcq"]Õ?+ÎëRW—?{)ÐuÀ…?k·;vhé¶?¥"ŽØ÷?…Zv~ù4FGL J2346.7+8008?èØÀ®[r—@1 -à
À9º¶åÚºÌÀ;ÍÂ5fê@¦7Õ.p+@…³ƒO«9?»(
æª?ÂK²›s8‡@iS×@úȗ^¿ïÿÀ_V&Ó?ïÿHkÇÏ¿äçøé
¿å÷BÂo¢¿èy‹!0Ò0¿ïþõÎÇúAGNbllWN B2344.2+7951?ïYêp•
??•ØóŠJ?±TšêÃt?)•º$Î?w¨£Ù£?q£"½Œ÷ž?íå~qÁ¨ï?°ª14°Eç?–/r)l™?¥,[P7?¦_ÛкÏ?¢'
›¶œ1?ìɗÌx©?¤Å6'•'?œŽM²)™?‹ðæÔ­|?¸ÕÔF? Â{få?é1þ‰5¯í?¥c°XVY?¹¶áÊhì?¢†ûþŒ‰b?¼¹)ëéï«?˜½úîÞ*4FGL J2347.0+5141?ïJñ=D"À#Ԕ-IgÀ8* Á@§À;h$Ÿòy@EY,ìó?ûñ«#.Ù1?lÊ{QE?¢µê!
Uˆ@TÀ%@hbå}rÇ?ïÿ5À+SÁ¿ºcCÇ* ¿×j[h†|¿Úï ^Å2O¿à
͞ƒä&¿×*kÄR{AGNbll3FGL J2347.0+51421ES 2344+514?¶,å??"¾Ì|[œp?36t^L?4rž©‰h?Ž>ÞÑÔOÄ?"u;©Ðäˆ?îÆô1Ò>'?ªEÎ;'žw?Nsʳ"b?`yVh`Ù>?£ð³±Iž?ª'Õ3Â?íÍ~Ø\®Ò?›Ÿ†ÄZ˜'?}ÄêyHÎd?u÷ )4ˆ2?¯ou+ù?™^ɋK
E?ï·
Œ?…‰Žoa¢ß?f‡¸É,4å?V‰CÒGÝ?™kR'Ù?"´
/­"<4FGL J2347.9+5436?é'ÂŽõ®Àƒ#5.À::sí7¦_À<4¨ÒÁ'@!†Š!×k?ù?yB=K?¾%ŸÌ¹–?È'?Š¤z@ÁvÂÔüF@RbŸ\|-¿ïÿéÅ+Ü?ï÷‰8ùEÒ?ꝡ»üñ¿ÔŸ4£ ®Œ¿×ՙd•€Û¿×n:%âeAGNbcu3FGL J2347.9+5436NVSS J234753+543627?êQ›˜Tn5?¼J‰ËˆÇL? B_±Ó!D?š"ñeìÕ?¨ù²9~á?¹v#¾þ²÷?讅×n?ɚÀiIœ?r	Dǂ9[?™Æñ;øž«?̵¡©¼~?ÉÔâ"?é['‰ëÊð?©ÔØFÓ?,/­-›Í?ÑÆ£ò?Æì/â« Æ?§Ã‹ñ›g±?ìˆ'HÒô?¡NèÁ~¨˜?‹Àêo¦‡‡?‡=O
ð?¸F¨ks? ¬!Z·»4FGL J2348.0-1630¿íBg‡è[
ÀQù2‹m†ìÀ82Îí8}À;]«›úœê@ݾ•Q‹c@QþÍ?¹? ãò¿`ä­?­H­Bî½
@T¿Z'È@Ïîq¸)'¿ÊÊ«õ¼°¿à.‡'?àÁ¿å&ŸÔœ$¿äì~ÃÕW¿è%Ë5ó×Ô¿é™ÝŒ7±AGNfsrq3FGL J2348.0-1630PKS 2345-16?N0ÚÓ?|éM1v­?9áÁ`¢»Å?2aĘBòg?†PÞhÄ5Í?|œÚÒ¿WO?ïÕ¤^Uœ»?{ýϤÐT?.dÂþú?HòWpYq?t=0BŠ$?yÕ_ð…?î灣þ ˜?Ž—Fr«ú|?vmx»hŽ`?oI$¶ s?tmQQɀ?‹ÉjvT?ïåfÐXÓ?X†QáV°?µšÀI?4²3ÿPt?i½Ô†ÚV£?XV³`Î4FGL J2348.1-4934?í
*¦OhÀPlvJßøÀ;,ägô À<¨¦¹<Í@‹>âéÅ?ý‡RÀ—4?ÞKþzÄÂ?åՏHÝ¿c@úÆ[¯S@	M/ê©V¦¿éf™£U¿äÀóEšN¿ånç´¯ ¿íc¯!–'Ê¿ïý³¿µ?ïûžaTƒ»AGNbcuPKS 2346-498?ï"/V.ª?'ÝnQln?_Ÿä5Rˎ?… ÷·?W…?‡?#Éûý?‹Ǧøé'?ï^™Ò%?¥"ì³ð#?rƒûµ1?Žj7H¯?šó-îùz=? 3ÚۙD?ì'›Çi&?¡u¼z_!þ?˜yCÛÄÍ?‰¾ÊtH?µQ*ÓµX?žÁ±WRÅ?ï+[Nšå?Šµ§¯üN?I떋W"?La÷3[…?™ÐwáÔ–?‰ß§	]4FGL J2348.3-6049¿Û"P{\[ÀKT¼M"ÉÀ;¼ZÔ–À=»µMTG@lR
¾Ú?ùžõ#-+²?ÞTñÿŒ<º?ÜÊ¡yaë­?ùã÷aËÍ@氛"Äÿã\ܯ˜ß_¿íQ±k뿸4Àüßå¿áõN€ìy¿àÓnÝ-m!¿ïÿ:=°AGNbcuPKS 2345-611?î˜WÔ)s»?§}—XÂö
?tÂíû#a™?s°¨s?£â$þX(?¦¬Ç3?ï'8Ÿ¸?›áê_Ö!Z?^ÌdGt=¢?q¤këßr?šâøTtÅ7?™!Îb›´?ìŠ[ýP>ù?¡uƒù—X?–ÃÈoB!?‰p~-?µü-ù¹w»?át®ÑžG?îìœ>ÿg¶?†FUvùÌ?9­'pŽs?60¶î0]Ÿ?¡áÁ죆?†'øi'È4FGL J2349.2+4535?ÿ1
"FÀ/ÒmÚÎîÀ:¥ub'¬À<
È°ÞZ@—"Òã]@"Âqÿø?°yÅhÕW?²öwÁ½o?ñ/N6ĸ+@
ªúý·¦J¿Ðõ"¡•'w¿áþ˜h¿äÊæ¾:Å¿âz?+Žú¿Õ£'{šÖ¿ïÿX¥³ƒPAGNbcuTXS 2346+453?ïÜ@vHªC?e8†<òÁ'?6ŠâûÑúÍ?-ý)3bjÉ?pw«í¾p?dï‰@ü?ïÍzåé?~‰y‰kC? –&ÄÇ1|?3²"žÆl?xïVåD?~,…‰s*€?ïí]0­m?ƒòýàž-?d~v¨[?`£~y×?›Ò…‰µFë?ƒàm¦X?ï®i¼¢?hqŸK¥ê?:â<ý>7?-Ÿ0ã?ƒŽ~ñZÐP?gÁs±	Y4FGL J2349.4+0534¿ÈN(yhCÀKo?Rü&À:`%t-ÏFÀ<KÏå†6@¡-g—>@ÕÓ;{×?¼ÿØè¹èD¿"©*±.‹¯?Ö%Â1hWØ@	â²r®?ïV%;"뽿éàp]‹ …¿ãßvó|d¿æwÿëÞ
¿ç…æ>7ô
¿ïÿÓ?,» AGNfsrqTXS 2346+052?ïÔM(|Íï?q'¾Q¨ôª?Eš`¼¢ÁS?<õ­Ë ‡ç?s&ª°–?p¡ÚkìµÞ?ï¤w=/?‡Ês±¦?5Þ%ºÕŒ?J¼…0¸×?†3?n	ˆ?‡Ý{~ûÀ?ïz±'?'œƒÚÒû)?h–õ_oÁU?Tõë-ì<v?šœñýáâù?¼Í—'?ïf¾žäå?rÃ*ŒÂ+§?YËx…Ñl¨?Gvvð³{Ú?'‹t›l©?r¾nª
4FGL J2350.6-3005¿Û¶(pŒ…ÀSA5Tu£À:#5'Ì÷À<k‰öŽg6@ÙZÂC[õ?ÿÅ%Ù®\Ÿ?¹U%¡OE? ¯&ɘdæ?ç?–¹‰$@\ü؃9[¿éµ³áC|W¿ßè|U»ô7¿ã×jµ€€¿Ù½Ü¡u0¿âf˱CÚJ¿Û²Ø
€ÇAGNbll3FGL J2350.4-3004LEDA 3231681?ïë"LìA?[l7k"Ý?(±¿_dñU?
Òm:ÉJ?bà—ìoE?Z,/} mŸ?ïÐuÀ$?jÿgHu4?)r˨?)?I×Im.þ?w'®Â¬?}Þ¸:ñ7?ïNñ}›¥í?y/Úã¾5t?`…=¹Pùî?Jßqo†c?"(•a#E?wñ9í)ïO?ïµêñiÕ?hú\Äfù"?8^•N‰j[?+ÊÊvâùÂ?õ™1?š?h‡ÿ$µ4FGL J2350.9-1416¿ïý²àJÀQ»y(àÉÚÀ;lmî$nÀ<ÉÎ	îü@]šÖZ•"?û6*^x[[?἖S"ûË?ÜH$".q?ù/H!×Á@~DÖHÌ¿ïÏBÈÒlI?ïòX!ªÍ¿ÛïY—Œ¿á\à
—2·¿â ¾z#³¿ïÿ>9 ²þAGNbcuNVSS J235111-141557?îjeñQ®?ÃFá›í£ï?iµ¢rNw?eæ¼ë¸?§¾FÈ÷`?ÃS,å=R?ï(Y€üW­?žgxUÚÞô?bÂâ¿¡ )?r¤Œs±¯?˜œsˆ€æP?œ9ÓÊÕ¤-?ì]ÝÎÒÛ?ŸœÅCàûŸ?žï"~(,?Žƒ3£Š°?µU¤O×!?™.º¹Ñ|Ä?í¹ê8ó?—Ø'½…&?bÇQY¹?e²ãøÙÉ?±¡f#jœ?—ŒEjjŠ4FGL J2351.3-7559?ïYŽß¯ÀDJ­ÕÀ­À:G,å;YÀ<d»±òUó@ iÐ~25?üµY~ —O?¸É­6Ú]?» ç¬!0§@HIёX@ØÔ2Ü?îöúÓpTý¿â¸§z¡‡¿ÑQÐb©~¿Þџše¿áú@¨f¼¿áz螺jÊAGNbll3FGL J2351.9-7601SUMSS J235115-760012?ïá~E¶§¯?_%鵩%?6Íϓ²?.y/CÚ*?kÀàeï‡?]^¿ww/	?ïTŽOŒ®E?"ÙÖB£EÊ?HßÀÍÏÚ?U"g.¤sÃ?"§8û¸•?"DÔg^8°?îñ5œ§Û?"ÝצƒI?hP`ðÅÁ?Va:ÚH¶v?žÏ@Lì-?ƒfóc'-P?a¬I?"?^Ëñ?wC•JØ?`Â9…%§?¤-‡3˜DÅ?'ùC³±X4FGL J2352.0+1750¿ï¢ò'røŠÀEd9¼º0À:¤Ó‰pÀ<\Ti
à"@T6üÁ\+?ÿ:F"bH?¼'uÆ«¡?ÀÚ™Z"†@gMú^ÖO@DVä"=	¿æK¿[o'¿áK+­,ôU¿à'ÉEnŸ¿ÚwPCKã¿éø@îݙ¿è,ì\µ½AGNbll3FGL J2352.0+1752CLASS J2352+1749?ïᢒzG#?d)ô+ܦ­?OršsÄÂ?J¼µ'Ec¾?f€Æèðí~?`0.wþÿû?ïu`eÑ&‡?Ó¹
½?C®Ýhè?VjèÒOah?¶'ÁÜCÖ?#œû¶e ?ï5f]"ô?~g¯ÏÚµ?j]¬a'?eDÒ
ƒ?–~ѝ1Y?z™q*²?ï&øì³Â?€K%uµÁ?e»'"Ê&?Sš³GDõ–?šã¼vî£?~Æü
Á‰‹4FGL J2352.9+3031?¼Ÿº@¿IÀ>®˜¹ZÀ;RƒZ'ôÀ<‡˜(€QÊ@¿§·¿tu@íx:¤?·Êóìn~¿¾\€^Š$@…ƒb°@È>¸w€??ïPz¼¿çwåê«%¿ä´þ¤á ¿ä0]ºpT¿è{~@w¿T¿ðAGNbcuMG3 J235254+3030?ï¦n9r¹?Š…£í[ÿ?hîžØòÆ?hù¶ê=£?€(ð»È4?ˆ¿r"ѯ?î>¹I"
R?¬m¥¡5aÿ?x<•ù³81?"ØÀ‡˜?©ا˜ÃÍ?§rrâïZ?î!J¹IËP?–¶Hé®?|ƾê?u¾ƒ›Xž?ªi€È
s?""ã].^ê?ê¯
z©,Ì?¬šÇð·o?'½åÞ×&Ç?Š93q\.Á?ÃY€g÷?«Î2ùÅ^¼4FGL J2353.1-4806?çxꔀLŽÀP‰VC´À:ÉÝÑôÀ<Å
?#@L£Ór¦@$É Èb?ô2â€hE?Á>Áh¼,?ü\e¬,CU@Oš"Ñ
Ÿ?ìÕ©ë të?·˜Jd°¿âzé«)äÖ¿Ü|Tú®1¿å`ºŠªéM¿âB¨@ÑVtAGNbcu3FGL J2353.3-48052MASS J23531112-4806045?ïsÝ´ž*©?€<xñÅ?ikÞ&î³?bŒ‡0m?Œ­Ï ë™À?}©†Ò‰g¼?ï…b"Û2v?Åƒô?OY¦=ÖÊ?aʔ½6qq?Œ±Üè…?ÅàhV+?î7
—Ð<?‰ó±æ?ußáʊ?båðlɬ?©ÞsZbè?ˆ0@dg³?ï˜1
Ú?~:‹D†.?y©»zœÈŠ?ee/°»½ù?–²7É?z´$¨h4FGL J2353.5+6646¿à½",Asà@&QßƤ•À9ëîÑÀ;'F1<¸î@½¡†øØ@õçB™Ø"?ÇéÀãàd¯?§ðd+´Ë?ã—cßM'ë@Áûa4Î>?ïþùÛ"Ðå¿Ùÿ€>Sοí5{!‰g¿ã^«‡ça¿é ÝZ¹‰ú¿Ô6ŽûçAGNbcu3FGL J2353.3+6639NVSS J235301+664243?ÌöIºQŽ?êA
±eç?˜èä·:×Ù?™Õ…añc¿?çû&k±èÞ?Ä«;£âjŽ?Þ@ܶùÍ?È/doé]? 4_\c?£ÿŒSL¹¼?߸—h[TÒ?ÆüV_Þe?ÕDaν"?®
 ÝXd?´êºó$É?–"+_‡Èm?âÀwº•¥?®÷zˆØC©?á'¸â«¾?°ªtþú? Ãû¡<µR?"8÷‰Õ§?Ûâ[Ø?°6nßIæç4FGL J2353.5-1457¿ïÉœ×¢ÐÀQö¨~8ëÀ;DâΖÑhÀ<Ÿþ­©@ (&VÉ@íÅjؼ?ŧRiÚ9G¿­eyxù?çþ)f*×D@÷»õ9'"?ïîX¾7,¿áËހ("Y¿êà*b)?ê¿Þ"aùð†¿¹ n†,¿ïÿÀéz-AGNbll1REX J235320-1458.9?ïIvऔÑ?•Ø¶zjXš?UkÛRøG?OE	¦Ö?•zf9˜6m?•†ò¬®£?ïX'mIá?•É8ö"
®?UÊ`þ?gk²×I?"¢J€jô?"*ÃêE‰?íF™Œo?™¹͒?v…õ:¡5?fÙxÂ),<?´g ‰‰:?˜lÃòþeø?í
§à¢Ö? Q¿vÜWV?aTðÖ¢4?_làºó	ã?¶:E×»? SÉ{@ÎÄ4FGL J2353.7-3037?µ‰^ÀS9Ϫ͞"À:7\óöÝBÀ<}:Y˜!Ê@ÇO"L«T@©3]$žE?¿¬Ð6f?¶a·U\ä?ö,û
͹\@¤Žèe¯‡?ï¦Á4éÙ¿ä?£ƒþ'¿Þx¹d»•¿à¡åÎ%'a¿êºM8—÷¿á4ÂkñAGNbll3FGL J2353.6-3037PKS 2351-309?îi«®ÁY3? +»ÚáD¿?Ïe'ª,—?™™¶b+â?¤ñk¯?á©?"ëjξ"s?ïòƧƒ? gI´ÖR?h^¸¡f5?uÁîʺu…?›UÐ*¾Hõ?'îð–ÏB?ìÆ)¶ßl?žslSÈ?š"W0"²?qŽü2Õû?³J.Ô|ûú?"Î+'ž "?íáÓíúù?_'× «?‹_y®#ch?v>©Ëÿ²3?«
â´Õgˆ?‹˜¯ÍM­4FGL J2353.8-3911?¼#0‹¬'ÀR?Až0PÀ;	æ~OÀ<Á|Ôfõ@ …±…@ïó»NH?ÑbäRzv?ÅVV"÷Q?óœ}YÇò@Æí­B?íü݀ú}¿é$â7˜¿ä=а‡é¿å^à
AL¿è5é
†¦¿ïÿþBe«+AGNbcu3FGL J2353.7-3911NVSS J235342-391442?ï—¶ÈGc?}²Óˆ¤Ži?ZØó©nõG?T܋#ÔD)?†ß³ØÀH$?{Ճ«71ð?ïAbª‡P?"ì²ß!C?W;9q*ïn?b®Üà@÷ý?–_÷(|g?"¼[Ø,Ik?íþxð?ˆ(z‹?'(á?sÆ% åv?«ØL'›ð?Œ§xâ#©?î0·éE¥?^¨ÎÅ×?qÁ;£öå?b¦^Ö-™o?ª¼h|ìÉ?àe É4FGL J2354.1+2720?æèé#ÎÀ@çu¸eÀ:ÖƞµbMÀ<›
ü³Df@x>He"@Òµþ,Á?ːßò?À)á¹mõ?ô}_Üßiˆ?ù§õ
j¿Ü°h}—ÛS¿á»'Á^Á¿æÒ<çè¿Æ6`y½[@¿îƒÏBrì1¿ïÿî' ÇAGNbll3FGL J2354.0+2722NVSS J235402+272328?ïW"|`?‰o=ä]ûˆ?`Æߚðê?X¾ÀÃVÓ}?'ö =2!Z?ˆ2Aõ¸¿?îZý¨VÂ?¦vhcÀÎ=?sþï¨úÌ?‡`·¿?§ÐG‰+R9?£*o4¾·Õ?î:§?Èìºû1?ƒåëÎþ
Å?zlú—2ù?ªڛ_<þ?‹ÒmÓVs|?íQ[1í?—ý£/}v?"P͂µ_T?‡>TðlyT?°c)ÅÃ?º?"óì}Ó`4FGL J2354.1-0958?sÊyÀQ
Ÿ¸fäÀ; ïܸÓÀ<|ùûA@ŸXŽâ[@²c"úÎ?Ða؂b›V?¼_õÞéÛ?íï8œÿ¨@Ý›ëÙW?î®X£/D'¿èÍ_ߎ›d¿æÆuÐfµA¿ØxÕÔ³K¿ë{¢´¿ïþaå£2AGNfsrqPMN J2354-0957?ï"XµÚ¬?'Œ…Õ¬%ª?TQ.n×¾t?J[ôUA>ý?Œ_ÔÄ®]1?ãL}àw?ïsi·€?l÷öO?O½W`פn?`‰tù݆y?"ÞaÖ²ú?Ž¿Ù'HÂ?î4âÜÃeÔ?Œ÷Y$Õ&ÿ?yþÍrš?k:4!)†?©r:%´z?Š[µ˜À÷?îÏï«>/î?…I»|
i?f)">e0?U¸ùk$?¡žm	µ?"ÐtÛ©§H4FGL J2354.6+4554?í¬l52gÀ/¬ÚQÎÀ:¤l™†NcÀ<pÈÜ}Cø@2êm·A@=Û?VW?È)Eßaô?Òð ÿê[@1o† ˜'?îo\k«¿íh­aÍz?ïÔÊ\°?¿åã$\֚¬¿çèŸ8iÿ¿àoUB§šc¿ïþÍ?äF'AGNfsrq3FGL J2354.1+46054C +45.51?îó¢|?™ºdÃ'6ÿ?£yÛ­/?'k>Äß´?˜º-¦Ï?"×PÇû-?æÏìGÒìù?È/Ímpã?ÂIQÔò?Âθ—U=h?¨ŽßZ
?»Ä	F˜d?ê—×ÕóC?¦HeñA°ª?¯±JZÂÕ?—z÷Íçy½?¿ªœ>£~? WVh¡i?âò<¶ÅÍ?²¨ãó¤Ði?ɨ€K[à?´894Dß!?ʎªŒë?«GLÜö@i4FGL J2354.9+8151?½0‹k·@39¸ºÇËÀ:*Ô2ò›"À<B€'،@D5݇…@ÝÊeê?¤?À.I¼ât?¶y<×Ì°?òF>¢‹±@®õt‹Ã¿Ð-lŸ»q±¿æHdˆ?Õ¿æ=ò^¬³¨¿è–6—k¿ëpù'7}E¿¸—ß/OúAGNfsrq3FGL J2355.5+8154S5 2353+81?ëån	1Ï*?´VŽ^…?'j¯å@:J?‡'£uðÃÔ?¼yã½!x?³/ô~Cœ?îϓ"7ƒˆ?œÂ"hØÇ?qd"NV²?{!¾zßè¹? Ú52¼÷@?™.Z{i	?ì×¢Y–Š?Wø!\L¯?"Ú"þÉM?…Ž.'«?´d¶s™a?—Ý͈:o?î!ýà6°S?Œ"(q?ŽÕùä\?u¸|ÉÖ?¦*º~ãÃ?‡"!M'(4FGL J2355.7-3351?ï3¤Ý
ÀSzž+ϒÀ:,ÊëK=À<™QþÐU@wnåhz@€öÍ0 ?µŸÍ»4I?Ÿ¼*¤T™Æ?ãa¬ÃB	@õÕt'!{¿Åì]÷,è¿æ*—MŽÿ¿æq?2oê¿çäû¨'k¿å#'@ßÄ ¿ïéþ¡[.ûAGNbcuNVSS J235538-335225?ïߒK<ç­?˜c ‡¾¯â?8×:úèi?T«*/g	Ì?mRÍc»D ?—ÿ¿B?ïÃF"Ür½?†€Vé<j,?4Æ¡ÀK—@?I¹·ó?}SuÁè?…w+bUV?ïEoúù?€0r £Ì?fCü+ÉÍ&?\+'íÈ5Ž?"‰8‡¤–?}jIv4 ý?ïàL¬a0?ZIû…Àõ?LøÜ×o?A¶Ùsž×1?hu¹ÚHÄ?Vv¸—{˂4FGL J2356.2+4036?Ìd]f|PÀ52¹¯æÀ:"ØÛÎÈPÀ<Z¾ÎÝHE@ =û¹tUg?þْx=(?·0t¼ëXS?ª\Šo…?ՆŸ Âg@ͅþ‡/	¿ï¡ºÃ.¾?ÿ (¿ã'! 
ҿٛÈ]|\ó¿â"c'0qb¿×ïHÂçp½AGNbll3FGL J2356.0+4037NVSS J235612+403648?ï½êƒàxÙ?rU"CRm¼?PtªÏó¸?F#Õ­9ç?} å–M?pÀ¬Ÿk‡™?ç&nŒ?Œåé8¤T?F˜¾6å?[-©Rá	?Š}<ª"Y•?ŠíEÒÆ(?í–$ øO?"ïHæ2­[?gó"·?r,µ"è=?±òÿ#N?'îÜ3Ì}?î
~ºQ©?ˆ'Þûiþ?…¢ÑLþ?qoÐ|µ/3?¢†sÁ7%9?"é]ø#,4FGL J2357.0-4840?Ìó©)ttÀP:ÎÄÀ:ꋨ?OÀ<È«Yµ}ü@—Ì±Éç?ÿ¸j1Í?ÅÑH#w)?ÁèN2'úC?ûq¹_ã•?úý¿é+ÿbKO¿ÝŸæ+]Ò¿ãµ…Q8¿ã"ñ10#´¿ÚNÖ½;ŠE¿ïÿÚ
¢ñ1AGNbcuPKS 2354-489?ïmî*œ\ä?‰¶+&²!?]÷ÕÆSSF?YN_:Ս]?b½P.d?ˆ¿oô¿€x?ï%§RÌy3?—É;£òí…?bŸý7gî)?k³k ÇÀ»?˜÷ÿƒÛÍ?–aXý™ì"?î0–†ÏF!?C'Qý?z;ZzfÉÙ?oÿ—A»O?©¯,C¾Ä§?Š€-%eq?íŒûü)¹<?–äÃõ€?~u"ü¶ÎŒ?p{	ÙÎÃ?±°ÍîæÉ@?–)"CYµ44FGL J2357.4-0152?è|p+¿ªÀNÏÝ~Ë·úÀ:z–ê'°qÀ<zô/è%@LN†öª@ñ*_Oð?ʪ¾ZO?´‹õÈ|Ü?ñ"4 ½@;ª%-?½¤Òݲù¿å_×5ÜZß¿àHBY@ãö¿è6±•+v¿è‹D× ef¿ïî¤"‰—ÄAGNbll3FGL J2357.3-0150PKS 2354-021?ïÑ
ž®?¬¥'ª¸ðá?\ 2g&•"?gt ¿×(2?šƒÛ‰YÀÙ?«IzwxV?ï²ÀM×Í?"Í"¶@Úw?5ßp*ÀÃ(?H#8²?' ñãI?"L"_
ÿS?îàÐ
ˆt?†ø13ˆ%?r'­¸c‰?i¸"ÄH›<?ŸER6-?"$ûÀÊàh?ï^ì¼?vvy
\c?^ø3*Hú?N1AóÊ?'N7lxd?uš/օ4FGL J2357.4-1718?ç—%屎óÀRˆÂß
A1À:;<ó¦UÀ<C³aÁ»ø@ ãÍJ 4©?úü´=Š?¿ÜhKBôq?©÷#́?îmÓ­'ž#?ù ¤äüD?ïÝÍ:°Õö¿ë>³>±@ª¿Ø}[À›<¿Åó.ö¸ƒ•¿Ýþ‰Þ:³Z¿Ö›V½ÑÝ-AGNbll3FGL J2357.4-1716RBS 2066?îûŽH/?"t¨
?Uî!Gó"?Lõo2'B?Ÿ?9ù·È"?"ŒDL¦Ý?ï5î^•à‰?™ª¯%Ö?`gVóÓGÊ?mÔo@4w?—5INɅ×?—žbØãæz?ììý¥Rä_?›ï'"—"?€BN€	q>?o@ý¡_*?¶Ég®Þ?šcíÿ«‡¶?êR{½íºŸ?¤û>$ã?ƒJ)õ5?rHèò?ńÜe©Â3?¤—Oy"'4FGL J2357.8-5311?îþ8
á¨ÀO
LÂPrÀ9³v/1EóÀ<B­Vœ@œÂ†!í'@…	¿œ?°1¶±W{g?"°Y_ÓáO?ߨ8ã÷5×@¨(#µ'È¿ÔDx $ο槹ž¿çK|€.8£¿æšD¿ë^œ£9UŒ¿ïÿëJwAGNfsrq3FGL J2357.8-5310PKS 2355-534?ïûrWÈ´?9fîã»:ž?#ÜûGUá?C'Åòè?=Mïž*¼?5ïË$<L?ïãò'@?uºˆ^‡<?".œˆ¨d?*aÖlcd?k‰·||±?tÇs…yG?ïD&7¢‹Ü?€$8ÜGp?j±ÐÌ_#à?bi†R¿d?"$þò"Ÿí?|¯z~ïˆ?ïû¾B.ö.?1bzG|[Y?x7õ#?ùý»=µß?>+mõ%?/"1^_¹d4FGL J2358.0-4601¿×f%õn<ÛÀQÇ%ÃßÀ:UŽ7£À<›£í°r#@üaŽQ@Õ8ü Ïï?¶Ml€—ü¿ !`!þ­p?ä)šÞh*·@f÷1OXX¿Ý§dŽu¿ä³[wN¿êeøí½]¿â¨¯à-¿áîKØE¦Ó¿ïÿ¢­>'AGNbcu3FGL J2358.0-4552PKS 2355-461?ïï'RêsI?j¨-iA˜B?7Þôk,õ?1…*K«&?[¹N.t?jjL;š?ïÝû5¢?v(8\‰¸Æ?3p=¿?1SYu`sA?q4´ðüÒ?u¸ø=¸ÕÐ?ïKkìsk½?}F¥Ë½=¹?cI>TGÖ?Qlԃ(Á?")Z§ŸU?{xüe?ïì\«¸®?P&՝-
¡?2me–%?$íìwb¬û?aVG¡ƒð—?NTð?ÃÖ4FGL J2358.1-2853¿èpš}!òLÀS‡óõ"À:dü'¶vIÀ<œBÇû¬´@ŸpÕ*>m@ žÛøº?Àv†š
‡Ó?Âø » ýÑ@}¡›Æš"?þYÖ)ÂÇ?؉хCKY?ꫦ!r™¿ç49ÀGƒ¿ÛÎó£PQ§¿ïÿ½_œr½?è[¨«AGNbcu3FGL J2358.3-2853PMN J2358-2853?î\ÄèàQÂ?¥—‹	C%?Ž$3º^?‹X,ѐj?¢ª¤¯LX?¢rþ,­æ?ì¬ï=,Hg?À'^ãm¥?¡¥Íªcx ?²•înj°?±ÅŸAlg?¶G–¢+S?ìn§/~å?žm謕?›L•Év"å?['');?µ·¡«2¢?•¹«¡Ãg?í'ÑwSo?T°»îÔ?¥™6^²±?–ZÃåv?¨OY<u?'èßgù34FGL J2358.3-1021¿Úƒd'`±ÀQE/Ÿ¾wÀ9Q}˜²
À<,ÄFŽ@jÉۀĶ@å:Ü?¯ÁðOÞº‹?µ\â?`ú'?þž"_¦XÅ@­Ô3É[(¿×Ų'¸#È¿ãðÝî]@M¿éR0^—ÿ¿ç2çHy–¿ìd¾ÆyÌ¿ÚäVÁ­´ÚAGNfsrq3FGL J2358.2-1022PKS 2355-106?ïârèd‰[?a=ã0R\q?@ì…Z\e?3x³Öæû?iiz Y?`Y	$r½/?ïэûß÷?~'\ùx6?0IÐøoÜ?VÕÑûr^-?v4eƒþ?{ø­éì@Ç?ïAǪæ¼9?z9ñ†é';?kRÅ궍?VFî"¿"??"\±ååÁù?wñëùYI?ïìËt',ö?Qƒ@Ã?9Þ']œ?.u.ƉV?_ñb?NÌb€O›4FGL J2358.3+3830?ÁH>)¨½EÀ72"áÉ´À: ôX,À<HÜ}Cø}@®Ö€Õ¨i@R:¸b²?»hŠØáƒ?'-c÷‡qµ?ÅŒ:
'Ö@
™dôÌE=?ïd' ÷¿ÙLo"È&J¿æ#׶ÿ†¿á'‡N={¿ÛMh=¬¿ê#¹B¬LûAGNbll3FGL J2358.5+3827B3 2355+382?ïÕ̞CKM?hh''ÜèÉ?>r.""·?0^0bϐ?s2öò?gUÊlVºW?ïÆcApÂ?~>^ÃÍ?)ÂË¿5q?=UÜDhsM?|IO%e?}ƒÀìZá ?ïu6Ó?'§¬™Að?g MäÌ<?Só3,qŸà?›=UUa+Þ?5
¸?ïn%.D‹è?q¸©¨rˆo?WŠ°£Äø?Cw÷ûîmî?Â¯-23?q–ÆÁæÌ4FGL J2358.5-1808¿ê¿ï]ŠÀR·D»ó¡À9Ø<Ç0«™À<<4ÿ¼
b@mS[?ýЋö–Ë?¸Š×´ÝAå?«à©^Ä£?õy²X­@@@tÁï•?ïä‹?Ž¶<?ÁK°B'—Ê¿àÞ¬É!F¢¿ÕçÓäC6¿ßMJ 4¨Ô¿åÎAvÂÔüAGNbll3FGL J2358.6-18091RXS J235836.3-180701?ïÅì©?œœÚPÈ?Nԋá*»¶?B¶ŸÍãB?Š!pÃb?~¿…á`(??ï©5ÑD'(?‡*Bé‹ÿ¢?:~iØ/
ë?MŒBØfG?"Þ˜`ý»?†tA&¢õ?îšÕԘ×d?Œ^ðõ/Ú?qaL9À?^ÃYrPöl?¤&y"ËQÐ?Šz4Ícþ?î¦uÈH+??‡ôáf¼ò?n–<"§?]"òØ2¡?£·Z´'?‡ ~X/4FGL J2359.0+3922?ÝeôC¼ËÖÀ6cÓ^·E|À:bylÓgòÀ<7g0Â@Â	O_@é~¿\¢?¿y$?`¤A¿'Å˞?ÑB>éÊ´@
M|'¹Ø¿âïãÂwß¿çѓÛêw¿âÄ´š¦ßÓ¿æ*Ac¿Þï2²¾.¿ðAGNfsrq3FGL J2358.9+3926B2 2356+39?ïÝÉb"º;?£$«`±B[?5²v×i³?,g¹ÅZÄ­?o€NXò?£%¦e?~?ïÐh'4¬7?{>j¯{? '[:y'?6«å+ó׳?wGًٸ?z™8I0è?ïD¶žBá?'Ž&£²¬×?l:Tc'ò¦?\ÿ–z`_!?špŸÇEƒ?€òþƒk½5?ï¦6¸³ØV?n¯¨®ÒžÈ?8‰Úڄ?*·o¨kz?…®ü5Éã?n™'ÞgH4FGL J2359.0-3038?ïÖ¨©éÀSŒSâÖÀ9ô·ˆ—é–À<;'&¶M/@ o"üT?üÈÄ3¡?´ ëóX§·?'«¥''"v?ßµ<ã5D@œåT-)?ïþé+0/¿ã'[ßú¦û¿Üôú¸îI¿Ô="_ÑKã¿ßQÞú¡Ç;¿Ó·'¸¬"XAGNbll3FGL J2359.3-3038H 2356-309?﮹lØ¿Å?yÊшRÆ?B·X'¾¨š?: ÃwUú?ƒ&/@´$N?xÍâ©Ð¬?6ž\?Š˜'"‡ð?BßòË7æs?XU¢¹O¿­?‡îs+µ{V?‰yÈ?rT?íGyø7¿,?˜Jj¡²¨ë?€tŽY¢Ñÿ?q̬ ®?³µžs
¬_?–ûVï°`?îvtȈ»?‰úI†~+?h@ïV'¨q?WpˆÕ»?§i¾Yê?‰L»F4FGL J2359.1+1719?ÑR#¬`#_ÀEâà"&þÀ;5áAÎ×iÀ<µÿÚ$@À€ŠÔÚ¸?þfv÷®!ç?Ë©…ïm·?ÅGФÕN?úÀâ³¾ß@¾ivf9¿ë‰¤>8Ió?ïìl5ç¿Ë7dpB¿å^"ñ¿×h@zi¿åƝ]É^ÙAGNbcuNVSS J235901+171926?ïT;:y0 ?ˆVZIΏë?añßçõ¹€?ZKþ€d±h?":\³ÛDî?‡ÿÞC?ï@¤Bœd?"ÐÁ>³aÕ?K¬6¿ ÷Ó?ZŠìDU?—3kÖ?"#éLW?îéW¸m?á¯Gþz6?|;ÖÉßƅ?nD)?¬P†'H€_?ŒÁiLzú?î·P<Ã#¡?…Êö'—jE?hX]sß?[žCc
"?£vZֈ?…`S¼J¬×4FGL J2359.2-3134¿àîė°F•ÀSsC¬ÄðÀ:Ê§XžþÀ<Œ5¶›2 @üЁ¸&x@¯¿%D]'?¾šòŠ ªÅ?£ÿk@Ñè|?â%Ûüëx‰@ÌÆ+$q¿±=´€û"	¿ãB©D1ˆ¿ê-b
ç¿æAµaÌ"Ù¿éKŸÀûs¿ïü{Eñ{ÙAGNfsrqPKS 2357-318?ïܑÎ\§?¥)+=a?\K–Säâ?—½72ì†$?eI±>?'X—CY'?ïÓ¨ŠU1Í?Ól Ž¡?#KÿŒŒ­f?B~ŒìÃE?u'ZÙ³¦?~⿧añ•?ï=ŽHJ?OöVæ®?fʗ]Ñ¡©?W^Çѽ?•tä|‰7?}XùAP??ïïÑQ_t?IçL¬¼Ä§?!¦Ê¢ô§?B‰½mf?^;Èûì¹R?I(À¯Ä-+4FGL J2359.3+0215¿íóâ¯{ÈÀM<ÿdύÀ;b:	ç
À<´a‹·@ ëþ±Ì@`?ù·ãÑÌ?Ó˛ÿûMi?Û—ßÛq@ó‡œAÇ@ÏÅwÃÜ?ïÝH°rùó¿ïÿóÀ¬ƒ?ïÿ¤Á	¿×¾?kOÚ3¿àÞ¾fØ|¿æzD5ëAGNbcu1RXS J235916.9+021505?ï5˜¬YÂÄ? Õˁ"Sù?c覤ro ?r_ô¢¦?–ÏÕ 9Y¼?žãhŸÈ~?îÛ*{}´©?¤SG 4À5?jß'{ºë?|§bœµ}K? ŸeÐi¢?¢zå… "Ö?ìU"µûÜî?¡¹pœŠ?ˆ—}ü0Ž[?yzOk-?ºCú›Ç? ®ê?‹lO?ê7O"¦?¬Š=ì©?pzU&¤)?m<~!Ê?ÅGP¹E?¬–*Ž§4FGL J2359.3-2049?ž¹
=¿«ÀS"¾7ޓŸÀ:Z€U$õƒÀ<‹³¢,@U¼!É(@øУñâ0?·ç
¶<h¿›€ØúÏáÍ?ä6wÁ½o@8¶Ñ"¿Û¯©ü=RÇ¿æ‰RÄÈòM¿âR°Ü¬=á¿Ý¡z¹"œ¿Üß!c'Å¿ÞÎÙAzHÆAGNbll3FGL J2359.5-2052TXS 2356-210?ïQtwóŸh?ˆéOM³€ù?\îì¹¾1±?PYJb«è?"'5ð/þ?‡Äš<îÝÝ?ï©¥Ȅ^?Š9
/r»2?6*ñà€E¼?M0:{?"åbþÚæv?‰Qo#ú4J?îäÕ²í4?[ù$Cà?xªcr@Wn?dê7ÝÍ?¬lf6‰!ä?Ž5ÓIF?ïiš!k=:?wqèÕî?T7ì\ð‡í?EÍÛ-+s?'‰=ÉP?w
4z4FGL J2359.9-3736?ïàËsöÀRºÛŸ'xÀ:òêÏS)À<ËR—|ˆè@8¦ÿ´?þ'5deÛ&?ÇrÀF׀?Т‰bñO@Ô×ãD8?ÿ‹O™Æ:7?ßð̆Uï÷?í\૦âW¿ÚdéÄTXG¿àJãq*¿éÓYG™ó¿×¸4½¤¼AGNbcu3FGL J0000.2-3738NVSS J000008-373819?ïÓphÿÚ?'Szÿžî?Š†ˆØäá?…qƒ¾…f?'M†mü×?ˆSÍï¸M?îf­Qà'
?¨ãÞ}»é·?"Žzÿ=×Þ?@HH†¦?¤qŒ"'iP?¤¥­>Ú¿?ìV™ÓÉý?Ÿæ4S.a_?¤NtFÙ?•Z2ìÅÐ?³Mƒ÷>C"?"Ÿà÷b
?íŒBêþÎÈ?•4œ;ƒLz?\{Þµ+?Œ+SÀe?¨­£#¸ö?Œ©mS"-4FGL J0002.8+6217¿ÞÒ¼ó2_¿ª!gâE­À8Áœ©'žÀ;^`¯m@u@Ý®Éü¹@‰øÜö¼?®'‹`òË?Übþ<†n@%C1T??ü±åÃhÊð?Áºg"ôq¿Æ|Í[g¿á©c;8»¿çBëØ*Îá¿ïFMä¬g¿ïÿÌ~sM€PSRPSR3FGL J0002.6+6218PSR J0002+6216?udõCãk8?®jZHƗ?î	AãLT¸?±ÏKµüÕ?¬¿C"¾G?¥9ÉíÏ>e?{{ƒËÒß?ƒõŸ(©ßœ?é¬EƵ`?Áe]$iV‡?ÈsÉ^™é?Á=Å o"?†îW°ïÛ?pÞuÿ-¡»?ìï=ý³2?™^n_6er?µ¨EdÎ?—Mä¼ö?Qƒ¡ê'?<´€ˆK?ëìÏ0u‰? o­@SŽ?À)¼³j$º? bÈʆS=4FGL J0007.0+7303?î¼,wh}~@$ìaR*o?À5'c;8»2À:xM'Ðÿa@.!|Òc?ý¯Qvëè?€"'—s¤'?ÑøÁ²½W@QTeâXO?ú$¸÷WåÅ¿ I[=¾QŠ¿É)ùù€´ñ¿Øör¸"@l¿àÏ>šõ9¿êˆ6šÆÀC¿î³'#iPSRPSR3FGL J0007.0+7302PSR J0007+7303?fwÅ-7uA?iPðݳ?î´@UèÄâ?ªfÊ"ÍRT?£T~N :‡?©³-OÐòØ?`•JP/?y™9ž¢¹?îý‹a%'?¸ùoMiùŽ?žLA2'½?¸Å{Gvƒ?®Êä£;æ÷?¡õ-mÐG?è+f`s'7?µq<Œ-—?ǟ­Udie?±Žnq;=0BvŽ²=oÉl¹qµ?ïü?®lÊ?Ué館?>Œ™ÓrÇ?Uéï¨ì4FGL J0023.4+0920¿»,'È~	ÀJrÁÁÖυÀ9›íQx™À<0j÷ŞÛ@…K2Åz?þ+O¤ƒ¨?¼J/¼P?ݞ7@.@¼æ")Æ@½f'|F¿æ‡Y%5C¯¿»,y@ïņ¿Ý‹ßœ³)Ž¿èqÊÛ[¿ëbœ!´/È¿ïû¾½?'PSRPSR3FGL J0023.4+0923PSR J0023+0923?¬8`\OÅ?¤º).ºû?ê>§.òYi?¾]-%Só@?À,†j?·ûë'[ú??µïëülõŸ?·ûNÂ	?él"²*?Â0`+·?¾²î!?¹s?¯ÊÊ⓿ð?žð¦ëÎüû?ézŸ®Átñ?®ÓÆáà&?Â"ΌU<>?¦vNÙ+ž#?ÌöÐóû#?¬®"oVYž?ÚfÊ}ûß?·îê… ñ?×Í–Ü?³Í7»n|4FGL J0030.4+0451?ïú{¹YåÀLÎi­BÃÊÀ7‹…º¿"À;‡^@'7|@Vÿë]0³?ü"µ—&"?š¶‡øºm?ÜzRõñ@?þº{'pÖ@¸wù
îF¿­@}Ú²z¿»Æ¤i¬A¿ÛŸv¼Ï)¿çŠ©Üݼ¿ît‰u_(¿ïþQ>¶ôôPSRPSR3FGL J0030.4+0451PSR J0030+0451?…ŠfN$^?š÷'õ.?îócîç¢Ö?±ŸQßãB?—¼ïä'ì?§›Œ½N?'1ºV!çU?¦'¹ ™?îTºËêrŸ?µ•:)Ä?¢vGâs?°gª&<÷ø?ž£
@¾NÃ?•.ùqÝ?ëÅc…0ÈÌ?¤˜[[Ì;?º, †J%ì? …Ø£8ù>¡˜DsÔíF>­œ'G£à?ï ¨"DiN?†ˆåLÑoy?‡Õ±
Ó݄?†ˆÆ¼Ú4FGL J0034.3-0534¿—b£®Þ^ÌÀQ³g ù	À8™¸Øú¹À<øä@bFg'A?ÿÕGª¹|Ž?¥=mbÈÂ?ÍیÙÝ@%Û°_®¼A?ûåÛÏI(é?¤7ÈÄ)¿Ô5Ñ>B¿áõ6þ™Îs¿æ^92¿í=¶y¤0Ì¿ïþ×@ÄnPSRPSR3FGL J0034.3-0534PSR J0034-0534?©BOî<
?£çR.èg¦?ç<'€aR?Çà.Û°)w?ÌÌ)j€7²?ÅøÆD^?¶dG·ã?ÃYÀBƒE?êÚ§7UEÑ?Çæ"\Ï
?²Æ*Aš?µD+"mñë?Ê"¯!â?¯¹ü2¢Ï?ã=äœy?µ¨›(¾Äf?ÇÇå¾ný?¬>»_Æ??¥ª8··?•yG€£®Ç?èáY|ÑBê?´û`¯Äwh?Çþ3l?±û‰Õ‹c4FGL J0101.1-6422?ímU&‰<æÀJ]c
'SÀ9nŸÀ<]
þÆD@3q¾‰=?ýút?¬î ‡—Æ?ÙÁ9d@+ß /µÐ1?ýMÌôåŗ?ïçlá)Ñ
¿Ï5¤&»V¿Ûò ›ìZ1¿ç"ò5<!ï¿ì«IúõÕ¿ïþó%&*6PSRPSR3FGL J0101.0-6422PSR J0101-6422?­)èoš…©?ª¹EI•?ëlâû]È?¾)^u£ïÍ?´ç¤°WÎê?´ÄW¨Ž>Ò?™ ð¼Œ?ƒ?›\ÖyF?í&¶Éuª?´˜´^¯?°'
…/Ÿû?±I	£n¬¦?Ž%Ä_'?ãáä¢_?ë¢};º½?¥…åp'¢:?»ˆŒ¶Êfñ?¢ÄG¤ù±?y¦Î"íòü?p·…!™3-?í®¬sZËÅ? SŒq´ß)?°ð/{ê­?žÁ{¹5U¸4FGL J0102.8+4839?æ"U¢7½À,VÏ d#–À8ê0IsçXÀ;Óg'Æ~@Ý«PÑ(Ò@:Ì}?¬¼FÓà?Ðàâ"@"Ëê¡ô²?þ
þÙy•?ïƒÂwß5¿ÑØ)ø!¿ÝãJ<º¿âàe0¿ëÈ°ÞY½¿ïÿ¶Ï4†PSRPSR3FGL J0102.8+4840PSR J0102+4839? ùòè2ú(? Qq'(îy?íTùs¤=?´v…wó);?©Å퀒Áþ?¬¡Õox}?¤xòhuã?¦8YŒ#¡?ì²;"ç×?´íå¬Í}b?°1ªÒ­Ï¯?®†ŽK8§?¶1SÇBUR?¨ÏJÀ÷%?éÖ
ôx-?±[ù¿öÂ?À"ýðŒô¡?£p%Ì/Ø?˜¡@Üã¼?€´öËQü
?él†9kCÅ?¦<ó6c=ë?ÇJ2ò7Tu?¥.51	P­4FGL J0106.4+4855?ïdöEZÀ+½í6´ÈÀ8©Œœ[úÀ;áiF·G@h'"ß-?ü#iüóÜ?ª]é?IA?Ýg.!üT$@/&VÍl.ý?ó½ÿšT‰?ê]»Çí¿¿EQîµ)î¿Õ™ –ö¿àçÉÉã¿î"Yáó¥¿ïþ¥AÃnÕPSRPSR3FGL J0106.5+4855PSR J0106+4855?Ž©úËو?F-±Eî~?ïLxη¦B?•ìś¸²6?|o£h•,?€c"B^1?ˆ2½ ZNª?'Mř*5 ?îX´E€Ûb?«ÉÒ¹³G?¤h_Û¶B?©Þ
>w?—¹åiƨ?np	z }?ìß»POÀ?œïÙMÐIj?³¬%ƒ×û?–öI¬[.Ù?&è%.»? ¨c#õÆ?îòÓdÎÝ?Œ-ÆaÁ{? »æ¤…
%?ŒÆ>a®ˆ4FGL J0205.7+6449?ÖCåCLl@¨Âa8ÿüÀ7n÷u³À;)®^L¼q@\íó@g™¼Õ?—Å
`¬?çQéßú@$wFˆz@ªIâøc¿­Èl뻥]¿à'5ÏŦ¿æ3ôÄb›¿èD¦ÃMÈ
¿ë~gä맃¿â²Áô+¶gPSRPSR3FGL J0205.5+6448PSR J0205+6449?ꯔúûš?¹}ؤ
Ô?¨!ß:õƒ¤?§ÿkäÒ?¾rh'½a[?³·ÌÀ;^î?ÒÃn5}H?Ô	~cš?ÙÊuœIÐ^?ÖëÜYž>?Ór.9Z?ЅÇùy=Ö?çŒq
Ʉ?²Tu~°K?»Öv6ɜ»?¦•_ÑIî?Ãã¹ue?ªõ#wl'?»^#h?¤yy"vìl?åN,X ƒ?¸_+²O}?ÍŸɧ?³øò¹{K4FGL J0218.1+4232?ÒJ¼úº'À1"~"ÐÝÀ7Â>Nh‡À;aHt
@¿égã5@ô¸ÙÐÁN?Ø›À˜ê{?Çjþс½@)ÆP¤]B@á+'¿Ñÿ']<9¿ß-˜T<¿ä9‹!0Ò0¿çW_ã?€¿í$¯ÂzäM¿ïÿŸ‡ð#êPSRPSR3FGL J0218.1+4233PSR J0218+4232?Ù'}YS6Í?Æx	R<ï
?Ö2±ÕÝ1?ÈÅLìP¡?Ð¥Ðёì?À'ZÜ#n"?Å©2§ÂŽ?Ï7$wHÏÛ?çÃUT0ÖØ?ÒËÀb9Z?¶".ù)Ä?½T¦®¾©ì?Þùm2飪?´ÀQt7¼?Ö>2£*/?´©NÔ®i¤?Åö©4ædN?ª:4x«#Ö?'‡%•-©X?'nã#e'¤?ê	í-ÞMâ?°!Mν±®?ŧf•áL?®ÜÌ©:‡74FGL J0248.4+6021?ÏáÕZîk·?æ­Ü|m8èÀ8>°C)JÀ;
ïunA&@Íx¤¥Â@c]$žDú?°¯8½5Õû?áUÛ¿-ý¿@"ž9'û@¤»üoý"¿Ú\DNŽƒ¿Ú_
Q'™Ë¿â°£¡ZX;¿êuŒ\š5¿ð?ðPSRPSR3FGL J0248.5+6022PSR J0248+6021?Åþ"¾?'ŸW"RH?íz5´¡…Õ?µqszq/	?°>Y›!m ?±çùGó¨?"$΃xc÷?®Du`®|?çKaS§|?Ín®'cj
?Ð6ðpy€ž?ÌnÑ˞H?šW¢ÔwOÊ?Šœ7T?À?éÕ×',õ"?«ëîu€N?Å]¯½?õ?ª"<V*>?c»ŒI…ã?U?"\/
?ë$üÓy5F?°[ÉU¾?Àõ‰?°1rÍ?³4FGL J0248.6+4230?í«Ï}i–À.£^·E|À;nµÀ@ÍÀ=%(H¦@S9›W3î@‹o"Ný?̓ÞC¢|?薈¢ÑPÀ@ˆšˆ¬âL?õ7xŠ*eÚ¿ïÿþR€ÖT?ïÿÿ>¹ú¿Ù¨ ½Ð/®¿áó¢Ÿ&ÌH¿ïÿwy´!¿î(zÝì¯ÁPSRPSR3FGL J0248.5+4232PSR J0248+4230?Ù̇ƒ²Ç£?Ëxñ¶·Š?áz™eÞÿü?Ëâ=À6§?©ò-"yÃ,?°=z0b?³Ž¤NæØÔ?¾·ÿÔEKþ?ë¥NQ?Â/ì6÷ ?®ÒQq6;?«ïÙ
…bî?Í/hÿs[?°IÑíY²Ç?âãù‰&ÜÉ?´ÂÓv¾8c?Ç@±Æe?§J£"pž?¤Œ[%ßò7?'Èsóvr\?íøý-m?)?œÉ\!y?—Ǥ˜6u?R଒F4FGL J0251.0+2605¿ïôÊùnÀ=~‹;26À:!["Ì´À<{¸;EPl@ÝgX(àõ?þ³°fd¸ç?×ɵÁ?äãkªs±@9à0Và@fw@(d"?íº@£^>z¿×÷½j.G¿Òn2b¨Á«¿æÜ>¯¾¿îú!~ÕÈõ¿ïû
ÝԇPSRPSR3FGL J0251.1+2603PSR J0251+26?'¯&뇮?''>ÎÞ?î}ûC~€?«Ì¨n0î?ž'p´*¨U?¨"õ¶A?ª/ï"J^?¨q^nïoÈ?ëG'I	›?¸Bsê¾Q¹?¸´Ý¿Eô?²$.ž=Š
?«h63v$?–fÉ
Ö9?êCSր¬?§bþò5E­?Àµ#ÈtM?¡Ît ±ß4?§ÌcÓ¹:Ê?Žˆ/Î55?è'‰M ³å?±ùE5§r¨?ÉnÁ֎á»?°QÖçõ54FGL J0307.8+7443?ï3´.è˜@,p&grÕàÀ8Ûö"o³íÀ<Gö-fÿ@aßÀšdp@ã!ž¶9?§ãÐÊ][Ñ?ã¾]~
qô@1õÜy@àTÍâ?Ò®íÞë2i?Õgá:Âõ¿Ö"ÛÅc!¿æ_f¿ï¯âjmÝ¿ïÿÞ§À£ÊPSRPSR3FGL J0308.0+7442PSR J0307+7443?j‹|Wè?vÅÚEW%?ïÕº›)í?Ù3ó®Ê?_uÜŒ?i»m¼?'ÉùÈú'×?œÇÙ¦\Ê?î:V'T?B?»ËŒ"+æ?§¨}gz?ºL?Ì73a?4ÁûP5?²"ú^ýï?íƒì0€?™S#ƍç,?°ž°«Ó¾?'&©C?
PуÈ?s#Ñ?ïß;¢g?e…"h]±?p(lSÆo?ezŠ›¹4FGL J0312.1-0921¿ï®:6Ì^­ÀJ/]$žDúÀ9ù…¤ðñÀ<ýdDM@JXE;st?ýίá»v?¾¿<ÁQnˆ?ãª)Ÿ5ºÍ@!»/fÊ@>Ï5ݲx¿ïÿÿÊPË?ïÿÿÊPË¿×,åÜhKC¿æÊ{ÿÒs¿ï*Aò闿ïÿö$´ë/PSRpsr3FGL J0312.1-0921PSR J0312-09?°à廵iö?«Û"SŸ2"?ì'ó?¶Ë–OI>P?¦KÿeúØ?±T¿•Æ?¥'ýഘ§?¨)Á¥Vt2?ëûu:¿h?»v
q¢2?µ[W9©¨v?·
ŽcÒ?©xsûR?—ÛÛÂån'?ëmg"?¥lqùW³?»]¥àE»? Ðt۞e?´®úÛ'? <¤^5R=?è‰m[h*Ú?²—åßj¥?ÂÍ$ѓ"?«Öì'Âù?4FGL J0318.2+0254¿éÂD6vð³ÀEË]9–ûÀ9ËɪiÀ<yÿ–M´¿@Ÿh#ÕÈ@lŸÞW8Ì?·Ô=À'o?â">¾°@ ã§Ú¤ý@–ÝàE{¿åC%ÿ˜üç¿Ç×±j¿×Ïxäl-¿äË»À5Ö¿ïÿúÁҝǿïÿÿ" 5•PSRPSR3FGL J0318.1+0252PSR J0318+0253?£¥ækîÔ?§Ö'›ã?DóNà?©PÏ®»V‹?uô*&áï!?xtI?—?¥ §2c?¢ÙŒ%¢[?ëé¯äàé?µ'ìW}£¤?¶"-?λ?±À~Dâ®?¢áf‹
s?"ñz˜'»?ìCg¹ –?6½Œè™?´tñÒö?"š—¢H'¥?°†ŒQ¶s:?™9+ U?é~‰ ØÖ?²¼ýwxT?Á•SÁmì?®žîa[¸J4FGL J0340.3+4130¿ï¢`–SûÀ&%kÊSvÀ8ªµr£ŒÀ;ö5©/8Ó@šV=#vþ?ûVAU4æ?§ÿ	µáMã?Û¨Ÿ{°Ðm@/ŽŽ}Ü¥?øŠi
/®Ä?ï¶úÀoÇ?–ôu=å¿Ì?€Êë¡¿àÔÀŒ!·¿ëÙ-ފf¿ðPSRPSR3FGL J0340.3+4130PSR J0340+4130?†ÍŸÐ@SÖ?Š´tj"+B?î{t•œö?ª.~zhbx?¢•Nºö¦?¥'Åݔ@»?"ÐYڊ?Œf hï?íl"i"aT?¶ò°Ñ
p??²Yº:?¶Ü,=?e˜?"ù‰Ð{"3?‰iHÝE,/?ìŸéךž?œ*¨¼¬U?¶T­$J?˜œËëK.?48Äœ‹=?/<§R"TÓ?îXaW?—îQ­è±¿?ªVxbˆ†?—Ó˜puˆÊ4FGL J0357.8+3204?êYÿ>[¡À0{ÃŽÀ7qJEžpÀ;…¸èz0@Oð}+#ð?ÿÜЅ¾ñB?š"éß,Jâ?â{+ðHÒØ@B~ÉÀ¨Ò@ÉD"'Ô0?¢Žmìl¥E¿Ê¾Iý$-‡¿ã#³In¿ìXœ¿úÙ¿ï»x¡§Z"¿ïÔ+Á#÷+PSRPSR3FGL J0357.9+3206PSR J0357+3205?j&PvL#à?pÍ鈨 ?ï·0e8q±?€aTU€ý¨?wT¥(¡?v@::în?ƒ»"Üÿ@Ó?+¬ô‡?îò*'å~Ê?«¤¸›*P?—ÜãTІj?¦5éSü?´žÀNHqé?£<"
Íî?êFký¥šÃ?©à™Ɩ|?¹-ßĊ¸? Ø×&4þD>dn` A">€HòT¬ª°?ïèüÉJŽ?h0'\?'ê?g"vUP¹?h0ëV)4FGL J0359.4+5414¿êǍÄèì'?ìR«~H…UÀ8¢xíÀ;€k©œF@۔œê@öß$¾%j?¯!ÇÐ䉂?Ý»Ÿíp±@'"M‹¤
'?ø…ê ²?Ö×Yƒ)Ì?äêÞÐÛOG¿àá@!X?¿æx'vµi¿ïDJ¢Ž-¿ïÿü9¡â=PSRPSR3FGL J0359.5+5413PSR J0359+5414? ß•Cðw?ÅABÙë¾N?îÿ5c~Ì?Å=bò2B?àî˯8l?£°X@†Àè?p0ÿé15˜?{j¿dÑc|?ëY<kúç?Àóáóˆ¦V?ÃyŠº?Àߛ€Aå?"¤gPîy?j,·\SCñ?íؐ«´b?–
$'ÝÏ~?´ôº
¸??"™<6¤Ãÿ?)K³BU?ô±½3ê?ï+"ΐ»€?…"Ú¬,'?šo<â5M¦?…zB…™Å4FGL J0437.2-4715¿Þ¡CØ®´ÀDû† ˜'\À8Ǽ_—?LÀ<F…½CÃ@¿bå¨eå@lBHyì?¨žÕ˜£O{?à™ä½¯M‹@1ђً÷ð@Cå²÷º?ÂÉ·Ùö€û¿Ô$¼øÄL¿ãþ´;Œ¿í^•a¦Ž¿ïÿØ'sâP¿ïó?B5.¶PSRPSR3FGL J0437.2-4713PSR J0437-4715?éY²¦ž?•J(K¡¿?îs*ú"#ó?«Rë¾æWg? X£"Šq¬?¢öNº4Q?•VŸåi'?¡)hú?í
Vu$Nj?¿ýA{Õ7j?²i6®ä2H?¾0ò¥:'?·Iz~>d?¦¨˜¯$;ÿ?鍠|áÝ?°KÙ6<Ë?¼Nx}ÚÓ´?¢Þ@áú?>"¹ï̶Ó?9-‡Gj?ïë™ñ\C?H:Òҝ?›èyÚDØ?'׀çã4FGL J0506.1+5028?åj­Ì'¦q@îcŠ	À:ÚD«*»•À<ÝR‹¾@ œKZÇ?þá='AŽ@?ÏÍseÓC‰?ïmß«÷@H±il«@"0ðÇ(?â
—Íç¿à¥Ã=×Ñä¿ÔÄAéã?µ¤Va
±à¿ìmc`!¨Ç¿ïÿ°_ïÉPSRpsrPSR J0506+50?ªýXo™Kß?¨ÿF
?ëX -Ù9ë?»pý#Õ ?·¼RYiŠ¸?´Óå»ð?—ȧ#>?§ÐC[ý¾a?çðuep?ˁÂ	$õ?Í]VË~{?É(»¢¤4?É«±½.É?ª ¼~k¤Œ?ägrÏyvc?±ãOa;V?Ķƒý÷­?¦S§dIªm?¤x¿ÚFÖQ? 2NO*Ϝ?ë¶ÂÆù©?º
<ÁÌ5 ?¸
‰Û‡‰?³üñªÁ6G4FGL J0514.6-4408¿Ð?ÔR
z"ÀA´^=¢ø¾À9ôËbi¤À<EÌòŒyö@Õ÷É$̓@X2%ìù"?¹R"¡?èԜ9‡
K@#W>«6z?ûÝr~øƒŠ?ïëý^åé~¿Ï͍çߢ½¿æhþ0Q׿ð?ð¿ïÿð ¼x—PSRPSR3FGL J0514.6-4406PSR J0514-4407?Ûb=þé?ËÛnÞ«?ÝU»š=c?Íc‡~ä?¾Ÿ‹0ŸÊ?·ö>xƒ¬?àJÒ4vÀo?ל¦ˆÐ?Õ6±ÎZt?×5`ºÔ?ÄgTˆIZ?ď¿þ"ê?א³7, «?²¤\$zRV?ىS
Q˜
?²¶'w}ó3?ÍËówŽ?¬[ޓu¡?ÓƔïlT?Æ1P_¤)4?À+§Þ.'Ò?Å´:ÈEÏ?âː¾5A?Ênٚ¡ò4FGL J0533.8+6800?îû#	DwS@2/À~à°¯À9j1ZëÞáÀ<`qªm@YZô˜B×?ý¢"#æ?²q¬?¹~f?×áäù~@#ûb(E@ÒÿZh¬<?ï½(êÚÔÍ¿ÓßZÃðÛ¿Õ³Üȃ<¿àŸÔçM"¿ì4 ñ|¯¿ïþ SPSRPSR3FGL J0534.0+6759PSR J0533+6759?µ_'g1D?¯9v&ÒTï?ìö.•.žé?±uaLåç?‡wÇ|.»Z?ƒ ¶">q?§Küàó	?³½ôàDo?ëç¯k@l?Ã<X[Ý?µö)-ƒ?»(äÑlË?§ç±ÅrWw?˜ÅLý´?ëÁ鈃ÿ?¡úõÅ)å?µüÚÙ-ìL?š/—Č?¬z(î³P?"Ò~=Õ?ë6	k{—¼?£õ´élÔ+?¸Gw«èu?VºŽwo4FGL J0534.5+2200¿æhfë5\rÀ ž³´ÎÀ4^ZXTÀ8u~¤˜Ñ@q?%3@¬À½ÊÑ?'
æÒ(ú?Êʖý'<@@ñ«!Z@GP÷iY¿É§•ßbÒ¿ÝÁíz—¿ãÑÖ!	e¿åÛ£>Þâú¿êô~ø-£§¿ïÿÛ¸"ÝPSRPSR3FGL J0534.5+2201PSR J0534+2200?²­ºÞ\'?´f#0{R†?ÞnûߏŒ?ЬòôU?Üæt\¨ÙO?ÐÒç'[Z?Ž¬4x›¢Ì?´Eĵ?ívÍbÉ4z?ÅÊòiWc?°tZ¢çÚ?‡æՈO²?Îðnë0?4?µ-ñ5RÇ?Ћ	õ6X9?³w¯+ì?ßü¾•1ˆ.?¹Âï	É«Ð>~Qඦv«>E¹5T§?ã
é›t4?ʋ¡'"ú?Ùê,OÐJ¾?ʋ ÈWVË4FGL J0540.3-6920¿ïÃëóa>½À?€¦—®ÞÀ8Pè¬&dÀ;1u§L	Ä@¸Ttvt@õV#"Cø?¥²žù)ø?ÔÆöôév@ ⟜èÙ@µ¬;ç%?îu×Ra̤¿änìF嗟¿ç	#•0~M¿çñbXdÆ¿ì6§â1¹¿î¤ZÝò%PSRPSRPSR J0540-6919?Ò
Ïi—q?¿øùN!H?Ё<ÛÙ?Â՚|>?Ýx¸U…|?ÃA\}00¸?¬z(Ž1.?­¢ÍÓQ¬?êåjðÓcï?ÀŒLR—?º—"2LI?¸´ù‡wã?Ö:Ì[yû?±ûóD"??Ӟðž†ë?°I_ÂR?Ö&Cé?± Üð¯l-? '2tKÚÚ?ƒ	ë+Hœ?âV*0mT?´@t?ž8?Ùí
]©û?³Á‰zì¬Y4FGL J0554.1+3107¿ïÿ¹ÛÐÃ@±@ìFÀ8²¥xÊìùÀ;êʉüm¤@Áj‹@êPÖ²(Ý?­áÀ,ˆþ?â+`kz¢^@+ýxÄ6ü?û£Z'"ÂÀ?ƒ¢=×üÖ«¿À.²šò_.¿ÝôÌÆÐ&¿éÞÿQš¿ïÿþBe«+?È^9Tš6PSRPSR3FGL J0554.1+3104PSR J0554+3107?hÔÀNŠ?kR`ô<wx?î~WÓMW?¬5-Ôûa`?¦˜õƒ>U?«%E8j
?ve»7˟È?€¯Îår80?ë*œƒ¼—?ϗjǛÜ?¢a°2°¤?ÃzÞÎèqg?–Œ0ôz?"aéÇaï?ë种Û? Ä"Ë\{J?»'¿·ZÒ¦?žÄ;³Ç\?%5ØßoD?5Íö<Ö?ïS΀ÃxŽ?†ñ•ä!­Ê?•[Ä5Ò?†ã¯aO·Ý4FGL J0605.1+3757¿Ä˜ÜÒ¡@ 
ˆ~¿#À9ÃÕ>ì¥À<'	µól@5&ƒwnL@ÖEüc"?»×²?>Ÿ?è¬kbNª@#ú<B¦m½@ý©¾Õ¾8¿ê§¼r¶?ï쎞"Ô^¿ÑU+@ªÀ¿æthAÝÅî¿ï{û#!m8?·!¶‰PSRPSR3FGL J0605.0+3756PSR J0605+3757?gçÞYP?a·í†k
£?ï–mùüª9?•BN‡téi?"Ÿ‰O›|?""½¿ðÌ?"
^«-Ë;?«6´¥GÛ?íI'»¸Ó?¼Ùð‡°Ð?°ðÒwmôg?·¦Ô8"Pa? ˜œ¿§Í?Œ€È±R¹?ìJE5ä€?šYo}Å?µaˆLÈ?"t¿@Qõ?q´é9¾Õ?^Þâï¨$?ïWhŽX«R?ƒ¾6qé?¥³æ‡&?'pC]~E4FGL J0610.2-2100?š#Ƙ 
À2.8ÅCÀ9¶òÔô¹À<cÅü-ã@LÏõv9B?ÿÍø`ÏM±?¶žÕ)g­?àB««êÔö@"%p£×
=?æ'rhÓ(1?ïû®Þ¿×UÌeHÚ¿Ý+'€Íoà¿æš._8õ•¿ïÿèM[Óe?è:Î*šÞPSRPSR3FGL J0610.2-2059PSR J0610-2100?Á³¨Ütnd?ÃxôAçÔ.?éAf>¼Î?Ç%ê:bÔt?²|Q24Í?µHz2[lç? Câ/º?®ÀüP
¡?íL'aT´Û?¶:0?Ö?ªó÷ºñø5?ª@¶D¡ã=?¥§#Žüç?"i!ÆLz?éâ6¥Ôh|?«"ĤV‡,?Ã
\"ï$E?¨àÔê%!?wz5ŠÖ&™?i¤>ð©l³?íAÌtUá?¢äpéâæ±?´{ÞC¯îš?¡ñ€ìØ4FGL J0613.7-0201¿ïïA¸X2À"œ-IfËÀ7ÿ6)‡¸ÇÀ;…ë¾íç@¢fè¾Æ@#¹…È+}? Ñê¡|šŽ?ҁÝ$Þ±§@/Qߗª¬?÷ÚöE¿Â1êžCøR¿Ôœ¼C'¦á¿áTaì""9¿å8@Ž:–¿ï
žT}‹¿ïþ{›Ñ&PSRPSR3FGL J0613.8-0201PSR J0613-0200?zk?Å>j?ulMâg	?æÔb¸ õæ?Æ̊\<1Í?Ñ퍏©%?ƏæÄåµ!?†]vCxt?"u˜?(	?ìmô8ë\~?¿-31!´?¹Ä¯pBí?½ûÈ]aSÝ?"ÿ>H
£?‰ÔäڟÞ?ë`ÄG–?§i,~Ã?¿ú+¾Ì™?¤½v†È?2TêP€$´?'ûN8¸²?í¿ír音?ž®,(m0?±î?~b'E?žŸdnt9z4FGL J0614.1-3329¿Ånû¢ð|ÍÀ5Óä öñÀ6åʅʯ¼À;7Äe>Š@æ]êÁÕM?ùkâqy¿ß?Ç+?ÉÅ?ÒÅq"tI@Db0<î?û‡"»c¿ø¸°W™¿§¶™bDÌ@¿ÕoiÚº M¿àz4CÔk'¿êD_½Õ¹¿î>¾L‰"PSRPSR3FGL J0614.1-3329PSR J0614-3329?Ä‹A⌍?ƒŽj¿Þ ?íñ/j\f?½/®Å,?µ‡åpË<?»(?þeȶ?¦æ±m?'˜b$ö[|?ï©Pê'	?¨CÕìPaÊ?•,)ٖ?¥í—å
?¹±sÄ?¤Š(úƒá?æß"ö?³x}Hödt?ËL*Ðù®?®Á.9›èQ>Pö÷q˜ë>mí%7Gh?ï©¥,‹&?×Á½Gw?…–²¾WŒ¯?×ƒ°ë4FGL J0621.2+2512?̼÷dQí@L–F(~À:õ۹ϚÀ<'¡Îò@û@ˆuZ 	 @mYO&®À?ÇéKó?ïÿÂWþė@ öHÇ@±B%¿â1؊p0ë?ìœÏCŸ'?¸¸Û¾­$f¿ÝèŠBŽšã¿ïìü‡7¿éL"b¥¼"PSRPSR3FGL J0621.0+2514PSR J0621+2514?"¦ï+D©D?†<Ë#@Ðk?íL4¦Ùtá?¶…|¥¯3ò?³	|ãËÃÏ?´öV†?ƒD¡<+?'‰5žÐHv?ëÚí7{†©?ÃK ƒ?¾À#BÃ6?Âf•Ïd?±ë#‡é'?•¨Þzb?èó*¹<?ªBŸ3ž{?Ã=ÃWÊG?¦Hâ$&@?kÚ.[ÈÙÝ?_Üø›È]?ïT†Î  M?‡­õÑá?'óàprÛ?…½Z@= 4FGL J0622.2+3749?ïôS'ç@%òµÖ\À8ÍIï7ZàÀ:¯ç¯§"@ìáÖõÈ@E!Whœ¢?±qta{Æ?êQ\1Y@1p æ)•%@þ¢vb?ÛÛPޔËT¿Ð*~CQäN¿ã¤©,´"ñ¿î€úfc¿ïÿîÝÃÀ	?ïrbS—WPSRPSR3FGL J0622.2+3747PSR J0622+3749?°"#(ÑW?¶3=Lߓ‡?êìÇ`I'?Ħ3՘£J?¸¾Úöh?½KGñÄ?'œ^ù}g?²Dõ£#ò?ìñŒ'…Ž¬?ÄÅsKj
?³Ì•"+B?Àtc£Ä¥û?¥Ê$ïð1?•?äß=í#?éXG"xÝ?ªèQ&֕Š?Å,Xsþ`~?¨3žðŒ´ƒ>ñÆJ)I>õ}À–7ýž?ìŠYà[#H?³¬òï?»¬ ÂC#?³ÃíÎè4FGL J0631.5+1036?´nËÔ?Ý`IôÀ83¦AGÈìÀ;qc´~ë@[áþ@и,+Ø?©%œq».?Ø 1ί%@+"ê»Ë?üg¿	ў?³½ŸˆF
%¿Çdëýi¢±¿ÙdÛ·K[H¿á~®üØ-S¿î œ˜Q›¿ïû¨¸Ž!PSRPSR3FGL J0631.5+1036PSR J0631+1036?z`Àæ¤8?wŒ¶˜‡!?îgºZKŒH?¦Õ!B¯?¦8B>r´p?¤©aÄZZ.?u½É¬~å?n¾$6©?ë=µ®"‰X?¾GÂŝXv?Â[:øMãw?¾ hÉ|â<?£Ï#Ô?"•¥"KÐ?íé©Å¾Î?˜/:Ý5Ów?³´P'¸%?"9ot¯¼?3Ì.ÑX{?%ëƒÓ4»à?î™hÔied?ŽÇ–BÏÖÁ?¦AÚ[ÆøÌ?Ž¹!¿s¬V4FGL J0631.8+0645¿ìcù-ö)à¿óêwTË3À8æpÆ;¹À;©´oÞµ-@Ây5v'@XºÍÆÈ?µúaŸF°?â.,Þ°O@"±P¹U÷ƒ?öT÷™Õ¿éâ—½#â?x6ŒGæ7¿ÎÁ ܙs"¿Þœ\W뉿í´bþQÿý¿å֔APSRPSRPSR J0631+0646?s%"ÛžK?p!."ú÷?íÕij*Q?´rCˈˁ?¶'"\`óŒ?³Íñ†ôG?z\?"l?PñHNv?é°ÍJŽ2Î?Áî´@`ë"?ÈièÙ.ùh?ÁÓH/\"?™­ÔÚ
µ?ˆÌd[Î?ëƒ
½
?£@ÎCé³?½|"µ~Ö? ­ÛO—d?KbeÊHQ?9èøÞv?í®>94Ãq?ŸÅL>›»ž?²WJŽOë?ŸoQ¸"14FGL J0633.7+0632¿ä)sÁI¿íµÕڒˆ-À7\Wï«À:¾çW'Ž
@W7•BœÞ@Oú Âî'?–{Ûî}̊?Øp;7äs@:@¿ã°>?þ;Ÿ]¨Ò?侏½wÅ3¿ÀfÌ}F§¯¿Üv" ‹Â¿å½ýûC¿íï@?5J¿ïÿäA2¥DPSRPSR3FGL J0633.7+0632PSR J0633+0632?3ª†–`•Î?.Ü¡täw¦?ï«;T¹?€¿Ëh¢ý?""ÖÉ)3?€m>ù ñ‹?e¿'Ùý?sbLU¹?íü,8
+è?±L–AQ¿?®áJŽªÃó?°°ü^›T?}Þm[:•€?bžg5µ—?ížRY@à?'LáÔe?±/†aZO¥?Ã§s}‰^>œUµ'd}>–MÞ"A?ïz]YÄm*?"OfDÑK_?´DùG€#?"O]@'V4FGL J0633.9+1746?íüý…b'+@‰I`œÀ3G9"†À9)`ì©áæ@ÄTÉ@gëC°Xù?hC˜ÚLª7?×&v î@l8²êò@µMÏÁžÆ?Àaäáìn©¿Ã2äá¿ÚD+]ÑÂU¿äØÍ÷o7Æ¿î>FVüf¿ïe<ã.PSRPSR3FGL J0633.9+1746PSR J0633+1746?VY
Dêª?Sc7³õã?ì¬éµQ­?¸ÇUÜQÛ?»©4}AÊ&?¸\ÍE?‡g5>å?¸A4Ù(ã™?îhÅë»=?ÄôófD]´?¡­uÖüe?À÷Ò!ñ?ˆöÑĊ?†:÷à•@?ëÎЂ\v"?ª=ƒ§Ö0?¾jª
¢Ù?¨â<þ t7ßè8"ç8‹`ÄGv?ïÿàH6ë?'#ÁS<h‡>ï·ýÉÖ?'#ÁS<hX4FGL J0646.4-5455?ë3Nô¸À6˜>·Ë³ÈÀ:º™I—#À<å³Ët9@áÞ¸1µ/?ý¤Uêî ?ÇïÂǺê?íuÉ næ@›ò9?ýJk±ò?ïøö‹â÷±?É|)WIh¿€|Àò+µ¿å…ؼÅÍ¿ïü¶ŸcÝö¿ïÞ?állPSRpsr3FGL J0646.4-5452PSR J0646-54?Å?ý¬ÕÀw?Áҋú|"*?è)l™d§?Äù
-°¾?´4ŸÞAYØ?³ˆº{_?©»Ò—Ý?©¢ì®÷¨›?ìJLï;?µœnî[æi?±!°?¯:8?¬{"‹xj?¾`ª[¯°?£ˆïe­£?è®»þû?«ž6w+´Z?ÀTðÖ<?¡58ÿõ?ž–ÿt«
¿?‰Ù'±ø"³?í€X÷R<?¡!ŸÙ#´'?¨®ðЊvê?™S*:RÍv4FGL J0652.9+4707?íIñNº@3¡/À:íu¶e';À=ÊC…Î@¾~ÜÿÊÑ@¥ð¿ñ7?ÒI·¤F›Æ?ïÿ³ß•ý-@[Ha˜¡L@,a$Wοã?ǖ,'?·†M¡sÙ¿ÑÄÌběP¿íðqJ¿æ´|¿Y=?–·Íûå­ÞPSRPSRPSR J0653+4706?Ö4Ü_Eò?Λ,ÿ˜?âïb6?ЛÅ?*cR?²@"rf‹?³ˆ¼*Ö]?ºÈw³'?·|<Ü9?êZ~†x?ś÷OH˜?²duWX²?¬
"MÛ?Ö¸ïã«i™?³¤¡Ûî?ÞüÊjk%?´ê–9ô×è?Ĕ‹cÒâÂ?£æ±KÖ?ÊHtÚ´P?·-‹q†¾?ç¹g@¦²?ºûþ£ªh?«Nû¸ŠÃ§?¢™Añ®}»4FGL J0659.7+1416?ïÿކwl¸@ ‰3ÁÎl	À8U×øyùÁÀ;¹SšÍv@ÝœRÜq@§-ä>ÙZ?§¾Ûrýœ?ߏã=Qš@)vB||R@}¿|ØÚ¿±A)¶2¿ä°Iÿ}y(¿ì~ð€±a¿ï4mÙw¿îøÛH'¿ï§­Ãó	wPSRPSR3FGL J0659.5+1414PSR J0659+1414?Ąc<4I?ǚrcÖAå?èÙvÏ~?ÏQ'§é%ß?¶NmÑw?Àþ"XÄ?¥@¸=ÕT·?ÁMŒ;…h?ìŽ6%˜‡?Æx6BREé?°îª/è't?½2-4ú´?ѽVðF(«?°Dű0 ?à~¯'Žo·?³0Æ 7å?ʊ"Õ9ïÎ?¬ê¯èì[o?V¶!ž?N˜×ÄÚ=ï?ïaª$?†Rðödw?'_]¬élE?…K©}«4FGL J0729.3-1445¿à«ò™‡rr?÷x¡Åg~À9Ä÷øËÀ;|rïá¤Ë@§>9Ìu@÷µ¼g?Ä1§—ß]?Á°å^"
?ùÖ‡å</@c‡8îß¿ï,ýäò³?ì-Óbh*¿ê°ü¢'‡®¿ã\áb0!¿è´y"P\9¿Ü~ÒÃܹ)PSRPSR3FGL J0729.7-1448PSR J0729-1448?ßìm¢µ?ÄùeFS¨?€m"#èÍ?w\:°'œ¦?ߐ*8ÑÅ?ÄèqÝ£2"?åƜ@‡q½?É~
Ž0@?|FåT·3?"ÖáSKQ#?Ô¯O[ɨ?Émô?á§\fŒ?·I°ç®‹)?¡TÞ}Ͷ'?‡pÂÍ÷Ô?ÚPdá|"?µó¢Ê计?çD¢á²èi?¤U¼J&Ž?¢¾ÛøÊ4?‡•"'#OA?Î=ìÂ6+Î?£ªóòÿ1
4FGL J0734.7-1559?íM:‹Ê¬•@')óÀ7Ít9ÀÀ;:¯ åS@³ËÉít@pM•ö?¢ž©_¨ß?ÑÒD2^ø@,ëXK±?ø¨©—h'忳ú§ü^¿Ú+ÎÛ쐿ã·'hÐy¿çpGüó¿í+/#:G¿ïÿå"m/®PSRPSR3FGL J0734.7-1558PSR J0734-1559?ƒ™m1è…á?€z¬ æˆ?êÃqg¶?¾E<Ø-2º?úgE8Ê?½)—¼@ÿ?}¾‡›ldø?‰
jӓBs?êH;õk§æ?ÄpaËÊ?Åñíuý>?ÃíÃt¬à?¥"nh""\?˜Î˯1?ê¤=ý†?«¿Þ-ÃÞ¿?Â,Sq£L?¦HuÜN;`?A¯£7ü?8¼RþDË?혶Œd'Z? Éi
מ£?³ìVmI.? ¹þA~ž4FGL J0741.0+6618?ànªáÔÇ@=ŸØ{V¸sÀ:{ÑEØÀ<›'BCJ@͜ùöPª@
U£ ƒ™?½Q°vÕÊ?ÕR%'@Ôà—"ì@3bt>kK¿çT¶:º¿Þ*ƒaHð4¿Û‹ç)oe¿ä'£+Ó¿ì–ÿ'èÒ¿ðPSRPSR3FGL J0740.8+6621PSR J0740+6620?ÝlMɹS?ćZ™òU?ށˆæbÅ?Ŏ#ñõ"‹?±ì.Y?Ÿ?¨¥÷hÞ}?é"¸4\?Ä~RcӔ\?»A$"OØ?ÀJp"lì?»©º
G1?¯™X<TÞ{?Ï,ŒêÀ'?³gqÛ!*Ø?ã®Âîn*	?¶)|>éÃy?Âg[‡8I?¢Ä¯Y>jÚ?èìã»Pš?¦¾ÏÚu·?¼Ê! b^Ñ? ]'0¹?»ÎÁ;i?›T'/4FGL J0742.8-2822?Ó-­€^è¡À‰p"XðÀ8êÃ×ZÅHÀ;¶–F(~@&(Ûì@è&ªŽ´c?±vÊâ'Û	?Ôýåÿ"àU@Ôñ€
|[?ýd"äÖ¯?êV?rÖÚ¿²khó¥T¿âTB)Æ"¿ç¡Y{•£¿íOx¾'²!¿ã#͚R&>PSRPSR3FGL J0742.7-2824PSR J0742-2822?r:GÚyl@?fn,[DŠø?ë•;E¼À?¶©QÛà?ÁÀÔA¢?¶,û;}?RkD¥	?–?ð]º¹Æ?ç§H"?ÄÈU'•kW?Ïq
9?m?Ä»¼Ç?ž·É³$§?Š¤Êp2Ֆ?ëN™uÉ ?¦‹Z؝Éù?¿§˜ïdéÖ?¢¨/Bh?‰­'/Üp<?mc4§·H?ì8M
|=ƒ? šº·\a;?»çf"…Û? rIò4FGL J0751.2+1808¿¶ÁAþº÷@5‰Å!ÞÀ9]oˆN»À<mByø¢@éR&ht‰@;ÔÂe?³²- ]iN?ç@Íàžö@+€Ïž8e@‡ùw¥¨ñ?ïÿ½OG"?驜œ€¿Äüì$Uõ«¿áà«aG¿îÉ=+¹É¿ïÿÈ¢› ÛPSRPSR3FGL J0751.2+1806PSR J0751+1807?'Ÿ ¹†n­?‹¨¼%.^{?Éz²{?–ŠMö·›?xyYϙä™?"ž¼@.õR?w¢Ðœf¼?'ní _ï?îø
B|Ÿ"?£`§ýW?›£‰k?¢ÊU/v¡?šxvQ‡?ŠÀ—‰.?ìUcD?¡œÕHç?¸×OˆKl?žîe±­¡?¬špöÜ?"tØa@|?ïÒéÂ!M?n™ƒ~Ǽ‰?vl–+<?nv½ µ4FGL J0835.3-4510?î*ÑØØÒGÀMCš‰ƒ¢À2{Èxª5ÉÀ8AA [À@ä¥}'ÿ@_ø"»ì«?gÖƒX/Y?Ô@Àæ"t@j¦[[Õ?øG>¾×?Ÿ
fÞõ¿Ñ``'çα¿àQúž—/\¿å£~IÜî¿ìö
Ù–ó¿îϼ5¥Ô:PSRPSR3FGL J0835.3-4510PSR J0835-4510?5£KyJ?3ø`z/µº?ïH&^ŒóY?œa®³¶ÊŸ?–§¡5"Ý?œ>(Ò[÷?‡=RóÈ?´7'Ýÿ|A?î×ö¨×?¿Û¹­´"Á?™yŒ;¤ºì?¶Ý;Ý:ãS?xKJžZ0y?f&Ü>jk?ì&ièC=?£C>iT`þ?½GüC?¢Ü33t[p8!T°kÄS%8byJQxS?ïÿøÛf?è¹ng¼>̒gõÁO?è¹nj
4FGL J0843.3+6712¿ï¦'ÍǕù@AÍÀÀ:hf9ñÀ<žSËY/F@Q¨¿&?û{Ɋ"-Q?¿-ý¿3?Þë¢ÐÏç@ªÉlÅü@Æfªƒø¿ç~è¾Dô§¿ÀB)Æ"¿ÆšXz"D¿×B¹ãæﹿé*æ}Íá¿ïðJ¶·ªPSRpsr3FGL J0843.4+6713PSR J0843+67?ÅNÕC#‹b?»pÜÖÑa?ê	® ~¡Í?½ )|g€?"S'×k7?"ÓÊ[¶®­?Ȋÿºv?ŎcsÄä­?æDÂ݀?É(èMf«?¼Ãñ
?²>/ù Ã?Ó^*ã3çø?°}}ªÀ‰K?âï…ÜT<o?²ºô؜Â?»%Ž|¨?ŸRNãœ?ՑøvúY?°½FÜ	Cã?ØèBŸ°""?µÌKµë?ц,gØq†?ªsޅôÃd4FGL J0908.7-4911?ïâãóϤ¿ï™–òö,À8‡oó­â&À:{ýÍpa@XŒ­@C\ƪsÜ?»Ì뀗.?à—-¾ªN@!iÓpô@ ôÆ/$?ïo5ýè΋¿ã6oÞ_Fb¿å–Ÿþ7©¿ìtáMK¿ëî‰J–ý¿ïþ}ÿŠ9TPSRPSR3FGL J0908.4-4916PSR J0908-4913?™ŠM_.ò÷?˜à±_ÅY)?ì%_ÿ˜¦Ï?½±)õ5c?¸rl«oË?ºÚ¶'òå?)›±'?š4ZÉە?ãyZŒ?ÌVÞbŸ]?ØÐsLÔßÑ?ËØðf†?¯÷áô٘©?œÃœz¾?ã4¬{w?¶«¬ä )c?ÔþšhmÞ®?´8`á¹û?VÜ?ÑÈ={?ExMüññ?ãëóŸ&?µ´•÷pà"?ÙÙKØïë‰?µ¦9ô†ø4FGL J0931.2-1906?îŐ &Ę@78ÿûÎBÀ;Ñ‹èÀ=nda©h@@¸MŽÔ@ºÃ.¾Y?ΦKÄ#°ß?ïûK€1È@æ…ý¢ý?ø^ Ò]…l¿ì"Ì3?ïïWq\?¶Q'ľ5…¿çVü\'¿íü'Ÿ½J¿ïæ#뗓/PSRPSR3FGL J0930.9-1904PSR J0931-1902?šG?Cx<?žÁ4!lÿÙ?î&÷ŸŒŠ?®,­ή	? læe{@Ë?£˜"ÚsÛx?ŽíàÌ<ý?""¼ú÷…à?î·
ihÌe?£wq)Ô?š»â€Tß?™Ë‰+^ç?À4cvXúü?¢'Z°K?çµÚIƒ€Í?®8ތÄ?Àô3c™Ó?£»½ó!ø?'XòËא]?s('{?ï[Syàšf?…<øØ6¤‹?†Ò.¼Ö#?€e»w14FGL J0941.1-5429?ރr®M¿ô‹'!¬ùÀ8úH…ªÏLÀ;µÛSñ@Þ)–|Y@Kh¢×0?»–ûÁÖz?âüÖö@"§â?$Øý@«<UEצ¿ïí×Äw"?ïÝ̙¡&V¿×?›ÜÀ¿æ{:ˆ&*¿îgý?[_¢¿ïÿýFKêPSRPSRPSR J0940-5428?¡v׈‡«0? æîÍH²â?î_r¯?¥ã3_&õ?'/¯ šÇ‡?P
N£ò¡?£ç–×u?»Z';¸+0?æÎAkK'ì?Ìö\‰c9?ÏâÀrlq?ÈƄ€á8ª?²ºE"?¡Ë,ëôÓ?êpè¨:9	?©ÚùÉǽý?¹¾§y+ª6?žú*«ZDõ?‡"'¡Ùs?q2?Ë®<ñ?íhöۀO?Ÿ"F9«§'?±ÅØÏÄG&?ž¾.½–á4FGL J0952.1-0607?È¥!Óörõ@A±tÿ†]}À:È5šì€À<ÇÃqÚ7ï@xJ7[·@#3vO¶?ÇqØõÏûU?åÑneZÎ@›"ªNô@¼½{¿í½FG.?ï«᛿Î">ï)¿åû«©g¿ïÿþÐñ?ïÚ?›Ü?PSRPSRPSR J0952-0607?Ɖπì¿?¿ëó2l´?é®ö3"ìß?Á%Dl"ÞL?™tëZþ7?•º¿sä_B?Ç|1Àdĵ?Å<À=³?æÐS²9Ì?Ț‰§`Ä?º"þï¨7?²?/ãIœ?Æêˆj¾r?®J#U4R¹?æ7éL½?³›ö`µN?À5ÒeU?¡ù'%XÌ?ÛX±Rv{?¸µÑöŠ›?ß™rö²?¹¸ÔÓ|=V?¶–ÔêMœþ?L}CGk¥4FGL J0955.4-6151?â@Y[³QÀø*ùÀ9ª¨ââ¸ÇÀ;ñ롤*@ŠÍ²¥Ú@ ` SÇþ?ºCSyO?ÔÐ=ºË˜o@»­ˆ["@ۄl5Þ3?ïZ° F\¿Ñ,b´€%¿á/âjmÝ¿æ:"ÀÅ¿íÎôÅ9Z•¿Û‹<¿N	"PSRPSR3FGL J0955.6-6148PSR J0955-6150?¢DÈ&F?'ÙŽWê¼?े¶Ç)Ö?ÆÐNŽy¥?ÜqÎiا‰?ÅXqö?¿‰Iÿ´'\?»¤až¹Ý¡?Ù/èÛHïÜ?ÉÖR݉Ö?ÞíĤÉïŒ?Éun¥ÏúH?¸sRێ2é? ™	Sýœ?å±0Ü\Ø¿?²"
m‹ ?Í" я?­|ñQƒ?ÒãßÆ )?¢àkÖJ?Ú ù£?©ïZ'?z?Ó	€7_ÝB?£ä]Tó4FGL J1012.1-4235¿ä;OŒZA@&u֝0'À:ˆ­¹OÀ<u¦N³Â:@,mÇ-Ñ@PwFˆz?¸c±€@,@?Ói^¾Q^í@»hH¾µ³@¬OТÅ<¿Öc[ïêß¿áöуòÖ¿ák#>ô\‰¿áSµõòð¿î¹ý‡»¢¿ïþ÷÷óÂPSRPSR3FGL J1012.0-4235PSR J1012-4235?Ï9ꤼ[?»ÜJ¨é6?åâ?À¥¯R§DØ?¹{mÇsX?«oCãgŒd?Î{¹CyT?Çÿ¾¹­ƒ@?áÁt>½ÒD?ÌᣱÒâ?Ê~uÁ'›?¸UMMŸ?Ñ$uŒ9Q­?±ýFXN‹?âFã›Ïj?³ÔI)þoõ?ĞÉYû?¢ù£|k	?Ú¨RÞš3?±j¥û=?Øʽͧ‰?³ôÑNm,?É"ÈA|‡?¯Îv%Æh4FGL J1016.3-5857?Í
'ºóË-¿þõ™t°¬À7dÿŽÀøƒÀ:;ƒo‹©@>ôŒÚ@cäõ8?©)·ßTä´?Ô°ß¼ÀL@$ŸÖ¶Zš€@'ð,¯?âã-ÌÁå?ç.ãBZ¤¿á×ûnÕ÷¿ålÚß4-"¿ì3Ô
2îj¿ïÿÞÝpˆÿPSRPSR3FGL J1016.3-5858PSR J1016-5857?VîÿY?Rˆ¾¹y¢?î\èb?¬"îE–D?¦w²?¬N¸-Öa?y6§a"ê?ªD?麊8{?¿x(gYK?ÈL!yäˆü?¿hãœÐ-\?ô>µŠ?'Iš.Q/ä?ê‹8£'55?¯ÓC0ô±\?Ãóّ©Ó?®Áåۑµ¼?>;÷žFNÂ?.l¶ˆŸ%4?ê^¥¹Òsì?©¦&K ݜ?ÆvKç
*?©œŠºßN4FGL J1019.8-5749?ݽÔü
¿åþ-BƒéÀ8u2_Μ±À:'
´©@ÿ¦|V@¬øCsW?¹Ü<ŒAí?Òhm
&Ú@Ýø?A^o?ú[çW´³?ï…/‡­¿è³ÿ ‡	¿ãíê‰v5ç¿ãØÇ«â¿ì:"å$²g¿ëDõÓVTPSRPSR3FGL J1020.0-5749PSR J1019-5749?•Ül°–Ö?Žùrâíå÷?ç|IÝö?¦_´uB™?Ё@¢ìÖ´?Âcå"TÍ?ŒÊ͝´SÛ?w¯Ï€üÒ?Ø!.ƒÃݎ?ÊJlëð¶?ã|=‡§?é?ÉýÈ)äŠ?°œ¢÷9ý*?'Û8èÁ¥í?ÜD©Zqé?´¹ôuøì?ߔȘ×Ì?³þñk©*?l#'ĘO?V'fšQ$ ?Ûè³
k^@?µúoúÚ??áïŸV"ŒH?µéÀ"zÃ4FGL J1023.0-5745?®ž°ý¿Ùv0¾ŽÆ'À6¦|µ]DÀ97Ó«ä@•#/Úä@W†Üþs8?¢äý› Ø=?ÖÐ6
Ù—@3hî9.÷?ön¼ÆÅKÏ¿Ì,û¡ ¡‹¿Ø …Üxfn¿ÕMý¹Ô¢"¿èq_=Ó¿íÇHɝmd¿æýsþÕ]•PSRPSR3FGL J1023.1-5745PSR J1023-5746?\ü
×÷Œ?Tܟcx"n?ÖPÿb|¡??Σ"<*™ô?äÉGÕ³›?Π?(÷‡À?hÙSŒÕ'è?u€]/?ëC%\'
?Â'løÍ8^?šZe?Â8	Ì?‡‰ÊÏ·®,?z+ˆä`ïž?æio3Ӎ?´ñã;¾™ƒ?ÒpÓAÛ(]?´†TֈÐp>£ãÏØÝw¼>¤
Z˜$?ìEC»í˜–?ª›]ÌRB?½ÕØ.«Nà?ª›X£Éaê4FGL J1024.5-0719?î.슊æ@D?_JsÀ:&­czù›À<nÌ¢Ûa»@²r'å¢?þ6"çƒ1x?Á …¸Ò?ÛÛO\¿l@Ô»ó¡M@'´ªA2?ì<+)yv¿àš®×ï?¾¿ÖrÆ{ÏÚ¿ãfŽàV¿ð¿ÕÉg}ΊPSRPSR3FGL J1024.6-0718PSR J1024-0719?ÛcB=ˆã?ÌiøÑ Ø?à·Î5›Ùã?ÍÄukíà?©iÄV¯?¤åÇ ›?Ä	3—Æ?¿±
 YÛ ?纁†¾-ð?Å[Öo#ã"?ºácõ`ò?²¡œÅpÜ?º>kj[?¡Ÿì&4ù!?èr`ò"A{?ªÛÔ'¬?ÁFolDè?¡‹¦½›k\?بŸ•yYÅ?±£r´dk?Ûl'©ËÈ?µ=ÆÔ4K"?Ç՛'ó´å?¤ÄãÒ¾Š4FGL J1028.5-5819¿åö¼¹šR¿ßz0ÓJjÀ6
\ËOÀ9ëQ=à5_@J.%'E•@%Uœê†ò?'Z,œ@=?ÑO>šõ@<g†ø­?ûð¢l¦òH?ë\âŽÕñ9¿×•Ù[%•'¿áåNšDº¿åu'¾´V¿ë«ä<U¿ï$à>ï~þPSRPSR3FGL J1028.4-5819PSR J1028-5819?pjè?­C?®PCò?펶]˜±õ?¸3ÒHñ~
?²ƒ¤4¶u€?³©'78ª?ap¬ÿ»›?wëÊBG³º?îzέ­ˆ?«PF0€¡o?§<JWƒb?ª¤ò;Ã?ŽÕ5¤"?€Aÿ>?éE­ä±:ž?±øÔõp·?É»àÍF?°×TE8>lIÇ[ˆ`>u¨‡›Ê?îÞVß7¿?—¾
vä?¢Gÿw¦?—¼›…~«4FGL J1035.4-6720?̘ü%Tù,À`n¹ªÀ8µØGTRhÀ<µ™ª`'@Œ<‹v–4@ÿ‹eú/Ü?©Àc‡ä»?ázM£÷Á@0o¸dàT?ùL•Xí,?ïöÎ}üÛ?͔àwN–¿ÖZÆ?iøA¿æžvx,¿îjÃê¥ü¿ïÿüoQÇsPSRPSR3FGL J1035.7-6720PSR J1035-6720?iz–Oç7?[Xë-W?ï܎ÃÈÇ?²Ô&Û—¿?›µ]ŠÛ?°ýÕ0¨1%?wÉ:¬OÅ?…4ý"Éí?ìW«Ù8…I?¼ñuÚîÊþ?»Æ
•Ô?¼'Šî¦?ŠqÀÊEj?sD†áȹ°?í8lý'n?–ÉõX"lk?´ˆ~Ê¿Q?•±Ö•>÷k…ZU`†>ð¨3f?ïÏÁÅFè?l'¡éT*w?x±×Ÿ¶Ç?l€‡L%w¢4FGL J1036.5-8318¿ì JhLÀ5'"»äG=À:Dã)/¤2À<‰æ¤å'7@óú0ÞP?þÿ ÜïYÀ?½ršÀúËR?àЍK­}|@Ž½'¬î
?ãq÷ÝØÊ¿î7ûþé?ïýÖZHŒ¿Àí ÂWÓÑ¿æ6™ºPÉF¿ìDŽ#ρ¿ïÿ®¡hšôPSRPSR3FGL J1036.0-8317PSR J1036-8317?È;ú‡Ë@j?Ò:¬Ôa8?é­	÷O"?Ò"¦¶S?€ýÙ¯‰Ô¢?…pñv¸ã?§'¤a];k?³œÓÈÅà?ì1š_® µ?ÀOwɸ@?²±ÚÑÜ\ž?³èÝìTK?­óóyÒ[?˜bùJZj?êòz úÂU?£ÐéüÉ?¹r1;¢(?ØaËÙé-?‰ã\¥ç1?w Œµ%zA?ì—
Œî¸œ?¦ö½úL—»?¸(ÍTð?¥p‡Ëk:4FGL J1044.4-5737¿èÇztT)'?ò€]£IEÄÀ6õ€ø¸ãâÀ:jýKð™[@Ôä'±@ΕY˜øŠ?œËux–Ùe?Ôb«Ü<Vr@4B†ƒ<`@J€y·üÜ¿¼3@®ñÅ¿Ûv·¢CC¿ã9Â~•1U¿ç
ŸÎ¿îYD_*‡é¿ïû•"d~PSRPSR3FGL J1044.5-5737PSR J1044-5737?X¤ñ.´Ë?UʇýjW~?í:MÊ­áÕ?¸'&?c£?µË*Ì6‰?¸jazRöû?ošÂn$Ó¥?w¡ØåÖC¤?訚ó" $?ÉèIéµ?Ìß)'øì!?Éç
¼<§?"™KN 0Û?ŒÿD:X\?ëtz8‹™7?§`
¯‰¼?¿uÛgû*
?¥#å…uI>ò'–¤¶Ìµ>öKùã …?읃¸äàå?§†ñ"K–?»ºn­q?§†ÃjR
4FGL J1048.2-5832¿š=p"êŽh?â^$ãåFÀ6_c-תÀ:?aÀxi@ýÊE³é@Ñ$šéû²?'[r¹ÓBT?Ò¦‰l$ìI@<"™(Z'@"›NÐrŸ?ï:$n:¿ÍõX‡*¬&¿â5¹ö0s¿åh2^L¥¿ìºr•;f¿î¥¿—°
PSRPSR3FGL J1048.2-5832PSR J1048-5832?2Ž¸%{ê?/Za& ޘ?ï!¦¨.Ù?•ð7]Õ9?›€ðäG}?•Ùßtò?a+-®K,,?pi_÷ÎEÿ?îd=e/s?­¿I:rÝÂ?¨©vÔØV,?­C+²P´Þ?.Oc2¢?p'—(ʏ?ìӋk¿j¶? ÔgÃGît?·=Ú¾ØD?ŸË¥þ¿.>x)ó¾G¤>)9krê}?ïMBí#žM?ˆüM2¡"?–WœTÁ¹}?ˆ÷1¶rÜ4FGL J1048.6+2340?ì5E½W›@O0¾
í)À:5¸H±JÀ<X•âTô@®°¬Õá@5^³¾?·ïðh]a…?É^KòK@
yT!ÀD(@ª¢€s?ãÛÀÛ|é¿ß‡¢u‹G¿ãwr'dÈ׿âðc	º"å¿ïÿBu?ïƯ²	ÒèPSRPSR3FGL J1048.6+2338PSR J1048+2339?écŸ`*'Š?½\µM5-"?Àäh¢©P¶?·ýµüü~F?³3¹XÒ@?©žiÃòÇ?éø•ü–œ?Ť‹#j•?µ¥´VKUš?¿LyD?º•£IÏõ…?µÍç%dDÿ?å"cetp!?±tc–w?Æ8«†ê;?¬ª"ÜÃzò?ÃuÆãD0@?¡{Ò65Õ?êr#cí¸º?¨Š7§|å?¸éÒ|?£†Ámªp†?³…Ò! ?˜6E²¢8·4FGL J1055.7-6028?ïʖYѶ¿çŽ2BrkWÀ8¬À¾¡'À;˜À¤ @SÃvŒÏ@*]Œú?·³%ë!!?ÔÀÎý(µ+@x_»Qz@êǧŽ?èþ2Ö!ª¿ãÒò䏿ÕØǁß=¾¿åÁßԍí¿ì•ªåò8¿äaSlŽž"PSRPSR3FGL J1055.8-6025PSR J1055-6028?|Ÿt.Ïh?u!ƒïnô?îø±¥íö?–î÷úÛ¹d?™ÂeR
"?"ùˆ·?"&WÍõ£¸?™€]±@V?àŒŸŽ´'?Ê)T¢?Ý´[fí<¤?ÉóRYVÚ?¡(øá>ø?Œ®Lj–?éW;y×?¯B«'Üê?Ç~LdÙÈä?«Èà ûA?ŠšF—à$(?qÀxT$éÙ?ä-Brâg?¹°$¥
Ý
?ÖЩ[:?¹c°¾4FGL J1056.9-5852?ís–r<?èîš|îhÀ9×AšÕÀ;Å<¤ËüÃ@?bØè9@ìåÜhKC?Áü	ÂÌn?ïÿæÀ
@"vsBí»?ö–£Þ S¿ïú˜i²?ïþW‰SÑ8¿Ò
è@EÀT¿ì2j€§ZL¿ïÿû-2h2¿ïÿ'¢."'PSRPSR3FGL J1056.7-5853PSR J1057-5851?•IßG´Á?¢ry•p+?íÐ]'½Q?¸1iOvúQ?¨x
H0P?³;¿t
á?xE²ˆÙ7?‰…zœy¢L?ìq¢Á~!Q?¼W¼ÝÑñ?ºîŽÒögè?»{qÂ{è÷?¬™ºö
?•±«²¼¹}?çàwç&á?­àhÒáÎ?ÉWÀs;¦ù?ªׅ¡e?‰ùs?ÊASÔ¦Ê?ï̬äÀ?qVIå†	œ?yžù˜:?q9P+]¤4FGL J1057.9-5227¿ïÕwxed@•ÜÆ?À5òtBÇüÀ:ÄëQóÛ@¿àqoXþ?ÿé}£~?†NY²×`Ø?áRqQ{ó–@TM)Ür\>@'Îunl?˪OŸO'
¿¸/g¡¤Õã¿Üà"È×˿钂¹ƒCí¿ï¤ƒ!Ýö@¿ïÿª9ú͑PSRPSR3FGL J1057.9-5227PSR J1057-5226?Qê²~(?QH¨¹ó?0Èè?ˆq$ƒ
+ü?ˆ =½‹–h?‡À >ž'?f^zäŒáµ?–	ǃÁí?îö!'Ñou?·mè/Â)-?žoþI@u!?´¬n"Ï¡¦?"tSbÐ?‹¿«"Bˆ?숗Y@Ô?Ÿµ0
Ü\ ?¶ž@#w0?š¹øUSIŒ<—ñ¤Ô°öb<ÄDÖÆ
è?ïþªTTªÇ?D#šhK?%ZºµS…Ñ?D#še4FGL J1102.4+0246?ïü"$(˜@K+J#9ÀìÀ;NVCÙs¤À=Y/F>©@b«@a¼þl'?Ô¬Ù<qËI?ïÿüÉï£@5‡†qž©@'H¿·e‡¿ìäšHì¿ÚØÐ;AI¡¿ÌoDö³¿ìoç¨m¿ïÿþˆ0»Š¿äðŽ¾^:PSRpsrPSR J1102+02?ìøÌCõ?ÁqÉV«¥¤?¬ÞYâ.j[?³- ~^-?°±¬Ð"?·Lñ³ï¨p?Ó°Nïê9\?ÎEÁÜßë?áÁíDI'?ÐósIZ?Á›&khª?¶Ågýqîi?äЍ=ó-×?±1µÚ?Ǝ¦[wl?¬Ò¿‰¢L'?Æ/$¬»Ü™?£z™‹ü<?ÓöìÔ?¹º3¸?ägMY²ª?½ç"pñF?³éå c]?©—©á«4FGL J1104.9-6037?Ö³5¶_ö¿ÚQ¡GãÄ`À8HzÿzŸÀ:Æ:¸b²@áTzU±@õ´'S+÷?²×f®µµ"?ܼñBM@"ëQX¸'ú?øß',꙼?êÃ'ëk¿Ó?¦n£¿ßÌ! Œœ¿å‹¡¿ï¿íBÞô¾¿ïÿÿ)@k*PSRPSR3FGL J1104.9-6036PSR J1105-6037?XW‹ãŽÈó?UX«+\à?'Ùµ@?†wßêwAÑ?ŠH ÖÐ?"l.gÂÂ1?u
1Á¤_Ï?·°Bé_Ù?é"èµ´ì?¾ŒENYöŸ?ÉŠÏ	Q?¾:üûC¯Ý?…Ó[»[
?p–Ør4?ìµK
3Þ¥?Y‡(?·›DjéŸt?šÑ'ÞÏ5b?0à"DÅ0?Û;ÈY?ëpôú›4?£xz¦Ôº?Â4(¥Q
O?£t¶Â˜)64FGL J1105.4-6108?¸ï••ý"˜¿ë˜<8dÀ8°8\gßãÀ:â¤itš@È(MQ@eº|h0k?»ÈÉ2
™F?Ôō]¡í@Y:´0ô•?ûÓÒ¥~Õ?ëtž½ÅÈͿӌÎû%OÆ¿ãê™fmó#¿çÔoŽ-TÍ¿ë€<01öó¿ïÿþ½à ¿PSRPSR3FGL J1105.2-6113PSR J1105-6107??fÌÈ´5?}~~¥–‡?îÄ|íÎH?´D]ÁŸÙ?¢³Þ}ðîz?´%éŸ\Z?ƒÛàzß=É?ˆQ¤
¡bµ?áSZ۞ÍE?ǯmá"?ܺkDëk†?Ƽ*›"ªj?¡oPÿóÔ?‹"^òèp§?çVãOÃoÀ?²nÛL?ÎH¬,²D?°'¹>ÆB6?c0d!$t?KëMæ«'Æ?æ5µµ÷¢o?¶žŒ'CËÌ?Ón3ËÎr;?¶'ù"Lµo4FGL J1111.8-6039¿Ú©=ó$ó¿¼$(ÿ'½ßÀ7—V¸sytÀ:'o™ëÎñ@ <|k‹iU@ËŲý?§hìÁ?Õgùä]K@*ß¼@ùý‡?åEfîVŠ¿ØÌï,¿Ø>("®zý¿ßw»B¶³Ü¿éêœ÷+°¿í'T·PSRPSR3FGL J1111.9-6038PSR J1111-6039?f§$…‰å?f<Ÿig»?ìá|РØ?·t:=ì·?¸>àVÌðw?¶ŽÆöhÜ?p†3žª9$?w´ —?èƒéQY7?Ä*ù•ˆ3?Ïe¾½ÅIZ?Ä#J,7>å?£D`¤L?Z?"79F"y?æD	T˜‰?´•¹ð5üö?ÑaCuG?³"³±vù¹?'ŽO6"fø?j‰ÂÏ2?çH'ÈU?±èoĔŒ?Ñl×0ˆ't?±~Jdš4FGL J1112.1-6108¿ãw/L¿á8­€¬7×À8•nÛí÷À:g µí7@ DØÒ³'@¨^=¢ø¾?ƪ^û'?Ͳ 8¯žê@RÎ-±ê?ñk	Ãù¨¿ê `þG™?ïKÄúpt¿çcÅ×惿ãíNL"-I¿ìTA ´@¿àÀ*ݤ5PSRPSR2FGL J1112.5-6105PSR J1112-6103?'f¯Ÿ6O?ŠæÙ"¢>¥?Ú¤±aã?Í£=ÏÚcå?â"¿w­œ•?ͨ˜ÔCC?…:Bå¥e*?'=òØ#
	?Ö±fÕø.?Êh¿Ù6/Ç?äœ>@þnU?ʘã'o?±R«¦ªõ¸?'ëè!;—S?Í)¯÷eÒ?¯'ÆOï}?æ‹>Q,Å?¯òԋ
N›?bÀF~AÐ?NvîÍZ¯º?Ù®0»ÝÆ?»]Œ	@-?ã'ƒÊ÷Û?»Q7¦æ#4FGL J1119.1-6127¿ïúû܄е¿áv"Ž¾À7܉ð¯*%À:ÀY‰QÞ@iœÄò7ë@J<d4]?¨ZàÜò?Å­7Ü_ï@;ÕýÍö˜@È¡Îï?âèˆ6ê?Ôkf€g™l¿ânE1by¿äärp_äl¿éBpˆ(X¿âÕð'3¡mPSRPSR3FGL J1119.1-6127PSR J1119-6127?¶#YåT'?©1¯l(ÖÑ?ÔÇƏ½?Ãñɉ[•¯?âØ
`X͏?Ãîq_7®¬?"ÖP?™™ƒ_á,?Ö0+Îr?ÌnÆgÔ&«?äCáÇjy?ÌWŒÈ¥é?ʎÔ4:ÇB?«þâ]]¡Ù?ÃîØ	©¼}?¦Ù+.>a¥?ä`"ð†ß?±"¿8FyY?š¦)‡eŠ*?émE0D¹?àMUPnOÓ?´ŒŠ63è¼?ݺòÆ­¹?³ùatltö4FGL J1124.0-3653?Ês	†€Q
@6ÁÁBá&À9#ˆ©[®À<JDÇ°-@óG;¨Í"?þOU!š"?¯Õ?Pç"?ÕÄ C@%dBAÃï®@¿é³¸SÄ?ïÿQŸ/пÊ
Þdú«'¿Ú¸©>Ó$€¿á'Þl	¿íR«ž~Ü¿ïûªÐù'7PSRPSR3FGL J1123.9-3653PSR J1124-3653?ž`­¹ß#?–—!
éÔ?î,ñ¶ršù?¦½n•¥Ó?œwÍ}²?›—d0?‹%&"{ˆ
?ŽÝ¶†@6m?î|jŒ›pß?¦XYë²?¡p
'*	?£¡¬H>?šŒ‹×¾'?ŒŸZ"‰?ë‡u¾VÐ?¥ƒž»s31?½$1\¨ï?£â×ãÅd?Š=!ÝÙÉ?t~b3ðÙÔ?ìœPæ»°&?™ë2X±à?·ÕԎg\
?˜°t®–4FGL J1124.7-5915¿ï¾–8f"õ?ü;V¸sytÀ7"^±f>ùÀ;ÔoX}p@!õÅ¿g_@_Á}ä1?!§"Kâà?ÎêõVÙ«'@(y!S6ß@-¨ìô-¿Ç®†»›w¿Üf9e&u`¿ä0&8xí¿èöÚQðœ¿ìÄw…¿ä®ÑnòüâPSRPSR3FGL J1124.5-5915PSR J1124-5916?3ÈWå?ˆȹa¡?çý%|ªõ?Ãî]íKT¨?ÎñsË@?Ã$§Å
×¢?'Ûh¢!?˜,¸¿~[Ô?è–v‹Ô–¢?È|£/uS?ÌxoF‹"'?ÈdƒHå"?· ©˜<Ĥ? ø½A]»?ã^{.Øí?´D¹7»?Ózß=ëû?°ÍŠóÄ}y?QÓ:ñ?CÍG½ÈÌ?ì˟Ò4(Ë?£'2ñ"Æ?¹[´ñvað?¢û¶å4FGL J1125.6-5825¿î°mJ[@À¥º9LRÀ9׋œ€ÕÀ<T›ñb®@ )c:âÔ÷@CüäŒØ?Àž":ê?᏾ˆfk@­'"ª?÷«]ƒé¯¿Ï"'ª>˜?ǗOýÄ;"¿Êµ_]]©)¿ÚHE¾ûþ¿¿íŒ*¢k¿ïÿ¬óéqHPSRPSR3FGL J1125.3-5824PSR J1125-5825?tØD¤àµ
?w<0ë•Å?ïyˆƒ¶ã?£+ó×÷g?–ú½ÆPöK? ûaìIÏ?~ZæÒiu~?¿rI2¼Å?æ:hZ܄‰?ϋsí–É?ÓîýQ?Ï2z'i²u?§Ÿé†'tC?—Cȁ.Ox?ë
êRÍýÔ?§H("z?»À¸¦GW?? e›C™—?~M«ìK|Å?hQñUvɂ?íÉ+2eP?¡}ž¸\|?¯£—\%{`? ÿËrY*4FGL J1126.4-6011¿í­Ñ\ÝY?îÅ2@QÀ:"ä;~[PÀ<?‰öŽg6@j­b#`­@Êþ§°´?ÑGAˆ
¦?æ²uhaé)@¤X9|ùP?ü÷s¼»1Å¿ïÿcW¾,÷?ïý(IË%-¿âÖ斢nT¿ác¿ø¨óª¿ïÿÙi"A'¿Õ›Ä¡Û¡PSRPSR3FGL J1125.6-6012PSR J1125-6014?Õu³Wª1€?Ц—¤v?ÚêÕ²-`?ÇQ<c0^?Ï@i¥GB>?ÂA_"? ç±Ü>?©²óh#?Ø}£]èdB?˺2{d?â²³?¾?ÌRð¢µû?܋ê~9?°‡~L}d?ÉáÀyTð?¦–™BÊ?փ5¾þz?­ˆ¹<{e?ª&ê¼kâÍ?•!èê?V?éi,[Ã}?¶tgœé?ÃєïuùZ?´slA=Š4FGL J1135.2-6055?°©Ë p'?Ⱃ`št‹À7Ð*o?RüÀ;4Ôóâ»@'±«^="@+¯EÓHè?¢XèàÞk?Ò<(…a9@&é䒼/Ç@>óp-?Ó3ÊnJ¶¿×M†00It¿áõÖ±R¿æà@è'œ&¿îiΛ&%¿ä±úƒ¿<ÁPSRPSR3FGL J1135.2-6054PSR J1135-6055?`Û1?ZÛq2[H?î=r9bèÊ?¦€:ŸV?«Lbô?¥ûƒé"?v'Zð×̪?|óeŽT?èÃ4ºa<Þ?Âìš}[?Ì?>ôN?ÂtøŒïs?'¸w^
hy?'óY‹›v?ë9}Á"¾?¥Øâ1y?Àâú.;ø?£•Í¢fa?M6½Üä?;äµ)qÉ?íA½xˆ7¬?Ÿ8V½d'?µ·§€Æâ?žö¾äÈ4FGL J1137.6+7527¿ï§²"z"@DeìÃã?À<ÝLvÑÀ=ž™Ó{<·@ ,Õöí@dÀĀÍñ?Õ¨ß<ÿí?æ÷]ßÚ¾@
Dr¦É¢?øçý%	O¿ï–­94?ïÿ—Yοо­dҒŠ¿ßv•¾BÆN¿ïÿ¹‰#)Ñ?·%—"0ÏPSRPSR3FGL J1136.1+7523PSR J1137+7528?ç)'ŠãŠ?Æj«Â?ÎÊûêú;?ÅÜÖþmCË?¢A—«9bl?¥õ[‡£?΄Ã>˜¶³?É¢¦*Î4?äÂ
÷?ϕY'#üJ?ÁѸós?·ù=?âç
³TÞ%?²nßV©ä?ÈI$iA÷?ª÷ZvCc?Ì¥CEu?«ÿŒ,XÂ&?š˜siŸû?§Ð~rü,£?éã–1è?±3ÉìE4?§dÏ:þh?¤bڝuÇ44FGL J1142.8+0120¿ì,tÓ´@Mµ\î À9Î{€©Þ‹À<F@îݘÍ@=5?§á?úñўå?¹Å‡Gw8?ՆhD7@P<«ù@ëpTü±—?ߟy'wéñ¿ÒcÀ"?h¿ÒTÑ]Ö¿ßÛAÖNV¿ëêòòÑCT¿è:"DÇPSRPSR3FGL J1142.9+0120PSR J1142+0119?¢`¡ØÕÉõ?—ð!™Sð~?í»˜÷WÛ
?¥H¿¡"{?¡åα¬…b?™Ý™ƒ—`G?ÅÊ\Û~i?Âs×&ª•?çrñâÙV?ƖäCs!"?¸Ó¸·r8y?±:ÿ
?®Æ&÷¨Ô½?ŸeOf†b?ë%«ãV ?¦& ™¨G?¸"¿%à¤?›V/9÷e?Ðã ÕÍN/?¬ÈJ ʧ?ژ'ù×lw?¹WŽŒ¡z†?Ԅ70[EZ?´kÐõƒ—4FGL J1152.0-6107?ëÈ$W´X?íwƒßóðþÀ95èºiúÀ;£ã³™ @XZÂnO@±æ­j1?¹œ÷rë:?سµÄÈqs@™eéŠs@HÑQkØ?èÎ{·?ïÚ&ò³c¿áªjÂkŸá¿çQ.ƼèS¿ï
¸Á?Èñ:j_kPSRPSR3FGL J1151.8-6108PSR J1151-6108?ˆœmidüp?…~<Ã
h?îI{$ô£C?£ñýž k8?¥A2V\Œ©? —Q^7)?'qoŸÏ?˜öˆ+% Œ?å;QD­‡r?Í]ôÏmW?Ôi4Ÿ÷?Ì­uÍ—f?­Åb}¥[ö?"KD,ÈÁ?æµ¥³0?´æ(ê³\?Ð9èdäôb?²yÈ??•;¼¹âwU?®¼OÙ]?ì`۞|j?©Xk s'?·ª3ݦnÛ?§Q'M'd4FGL J1207.4-5050?ë)B2´'@&՚•BÀ:Ô©: À<€`mþá@M˜f"³@ˆÌ»ÑÓ?¿Úø‰"ò?䂓=_ @E"¼»Ò@»ž`²?ë­2h2?ïÆÖÖ¿Õ^ü· =¿åÜá­¿îXO·Î8¿ïÿ™"{UPSRPSR3FGL J1207.2-5052PSR J1207-5050?r˜Ýq8Ñ?sxÃ1³Óý?ïÅ+B:ô?ƒä¿Jús?fŵâ™Û?|ڀ*"8ò?™¹±á¥¸å?£+想^³?ìŽ/‹]§|?¾"9©‰"7?µ ,©Uì?ºqô›…/ë?¥B'í(?'1×_?ì	ؼòcw?žSƒè,Ç?µð¡Øۈ?"o¿+I§?¡ì̲}?}KˆˆP?î¦-Œë¦?"Lœ·'¡?š˜a•íÔ°?—˜·/×4FGL J1208.2-6237¿ìž§ ö㪿Ʃ¸J´¯À7ýùp™ÆÀ:'Ӂô@ùx}À?@'í»YÝÂ?°jýNõ±r?Сzäw¹J@ ™íZáÍæ?ÿÏ懳é¿íå`³I?îïV.྿ãäÅø¿ä9€ô¿ì[`®–€à¿ì•†z$PSRPSR3FGL J1208.4-6239PSR J1208-6238?h™äŽ24_?fž~µn4%?ïLwý"D?–G¥/ þâ?"iôn•q?"€³õýc?ubwV?{n‹Î/??ç]4ÏxI?Ås¢A}½î?с»º@Ák?Åi	á°7ß?œín.[jê?Š@q—É´?ç‰þº(?²1`ìž'Ù?Î=úBª?°kï=fÝÏ?QéPص›â?@¹ ­qíÑ?è<"Þ—Þ•?³O/Œ®ÀÍ?Îêãït?³C±Íä4FGL J1221.4-0634?èËF=¸-•@KÂFŸ¸À9Ûò¿¥œÝÀ<E¿çáü	@îFïÿ@‡ü¹#£?¹_ !·"?ÕîžÄ%ß8@0T9=@dø7^»ø¿Öǁ¿gR¿ÖÌP:ªö¹¿Þ²«£Ý?a¿å{ºÁ1Ž¿îPüD‰¿ÂVjoàb¬PSRPSR3FGL J1221.5-0632PSR J1221-0633?«ÿãÓ$ú??¢ø"‹ùì?ën¦¶‰1[?¸:¦xPVø?¶ŠØb#ø?±x‹~‡Fœ?Ò!˜Ó=ÞC?ȉ¯X¯Â"?ãhEWþ?Ë m–R%ú?¿l±pÝÇ?²ï--nâ?°¢ö5?›œô?éîÅÿ-ê?§4ïèPtý?ÀA–ø;½? /Ñíi?à$V¿Æ?±—Êó?Ô+™o	Át?²гcVÎ?Çs%¡~?£ &
þ=(4FGL J1228.0-4853¿ë¶äªRé @+Hˆ/À8ƒ—‰!SÀ;gFvš@ÛýlR@,M€¼S?¦|)`y	?ÉDã^߉@rT¶"¥@<Y¹YÓ[?ï®K75÷3¿æ4€ãÀ.¿âb·O
¿å¢•Ä¿êá,À¨QB¿ïÿ}ß(ïãPSRPSR3FGL J1227.9-4854PSR J1227-4853?îiÅá\§?§Bqš^17?£i·©•?¥Æ V?‡ê<Ê1ã&?"×-ÓÍÒL?âƒöŒŒï
?ÔS¹¹ST¤?ѨĿ²?ÑÓj½‡?ÃÌÔEÂÄi?ÂÌ/K‹|˜?èZ¤Ah'l?²¢A1át?ÂÍl4o2é?¬ÒJB±a"?·‹à^È?¡èD"™Ã?Ó<f¾ùy?°wÆ`±·À?Ô·^÷¹
¢?´Ù~TÜ?Ø:IMÝä?·r»¢›Lº4FGL J1231.1-1412?ï3¥-˜áÛ@H0!¼jÀ7[ñ˜^À;WÔGëQ@Ú¸æ;é?ù—¡øìx?"äùБ?Ûü}¿sré@G1ïÝëÙ@	÷ï†á>?Ô½C¢—7?š¤^ˆeXŽ¿ÔŒËÀ]RÁ¿ã†€¸!D¿íîˆwÆ¿ïÿÿ&¦³PSRPSR3FGL J1231.2-1411PSR J1231-1411?½'C,%?Àhʟ>?ì	4Âÿ?ÁA>ίé?1ˆµßÂ|?‹‡lï xV?Ž¢f–ýÈ?²ˆˆ)Áß0?îÐ8ðuS>?»LÂÆò?–§Ó¾
€?®ü¶J%GÙ?»B)–,¯N?¦q)‰<ß|?é7
%J~?¬,Ľ¬?¸T¨üÇ?¡™ýŽ.®>#\æT2Þ>BHžl.LÚ?ïï.
$¥*?eKÉÔJ.ä?`Ñô¥šUè?eKÈì´c4FGL J1253.3-5816¿—&JA—¤ø@Y˜*ŽÀ:0%™È"À<
9¶Úó@Z¾bѱc@C'ŸÐ€?Ó ¡ ¤%?鍺}¿ÉY@
}œãÐõ@ÀÁ­§n?ëˆGô·M¿·á(V¶E¿éü…%Ä¿êÍñŪ™œ¿ð?ïÿüÉï£PSRpsrPSR J1253-5820?ÚÂìv0?Æ»k»¦n#?Ù'˜pë?ÉFK–«Y?È[×ãÓÈ?ÀÔÀË¡n?È׆A…ùÔ?ʉIy$Ä?Ú,
ý7úd?ÏqQEæ-Î?Ùh.â´?Í'-bY¨?׫À>@¢Ç?¬6±"ƒpe?Î!ʚ²P?¬Ìßªl?ÙC¾Ür?«;AÆÃp?ÂQ9션•?¯Û¤Ñב`?åÝZù+d©?»<¶W½Â|?Æ9Z.ÌÔÄ?±»`×­[4FGL J1301.6+0834¿ïd&}ÀÚ@Q҄ßÎ1QÀ9¨b/ ¼À<[å¯ò¡s@íJÛp~˜?þÚÙÕÉˑ?µ`J~ºW?ÚLó£¦7ã@ ÇTŸ"…^@^¨¯à?ÓÙp^·ÆU¿ÉÉ<Ê`¶Ï¿Ý"€ÐÊÞ¿å£ü~Á&&¿ï
ý˜F³¿ïÿ±[W>«PSRPSR3FGL J1301.6+0832PSR J1301+0833?¢·¢5íê?¡­ŽLü7?íÞ;ÜÛ¤?ªäòÖóH?žÉ[Xˆ·h?ž™ ôÃ5?²š*ïWK?½õ§Ã¸Õ	?ëè¤_Q?Â	ó*™'?¬AhÌA?ªÍ·Pªª\?©EÇyŸ	â?›=5ã1½?ëh
k›s?¥Mèý%Ë?¸ÈêsŸx?œÒm›£#?³}þʓZ?²¿åϜ÷?ézÄÊGϱ?°Âi
E?ÀUíq—:?¦ž'^Ø4FGL J1302.4-3258¿äŸ… '/ß@=ØOãm"BÀ9>³"&jÎÀ</#qõâ@¬–"¨q?ú£2ü¬Ž?´ä!s€?áì(¢‹…°@(žZWdjä?ò–"VŽ­¿ÖZE›ÀS¿Ä½¯¸ê¬¿É€Äápó³¿à%°"±"L¿ít0Ôý¿ïþ/{ÎSPSRPSR3FGL J1302.3-3259PSR J1302-3258?"=q2úɏ?—ܬA‡äë?îÓèæ°æ×?¥¦éo³2?'Eqöè["?—²mˆÃtf?€É©Õ?Š¯õ›xáã?îúöݙn?£—†±¬ä?˜<Ÿø'™?ŸYøPíð?Ÿ±ù=l²ú?'¹q,Eù›?ì%1öP'?¢)ʁ™1?¶éñþ Ã? ןX?Qت:8Œ`?Bät2Ûë!?íøŒ‰BR®?™…Ýw®?¯èr	Û?™7á>%ò4FGL J1304.4+1203?ä¼TL»øó@R¨¬1'À;cجëÀ<ñI{t¥@?Ž7£@2[úҙ•?Ï}$"®?ïfAý{k@<o"͊b?üw­ñ•Y¿êÕ>¶I(¿à»J>³‡¿ÁW)‡Óh¿ëìÀ|ÝK¿ïÿ>ñØJ?àæ.¢=PSRpsr3FGL J1304.6+1200PSR J1304+12?¾ì̃¼Íò?¸ÎÓy3hÛ?è'Vºß‹?Å`Þ{÷±?ÀOTc6Ý?¾ióˆJml?°<»n"‰(?ºžYÆш?ì!¦tŒùÊ?Ã$»x?­l!Ú'Q?´<BÊl]?Ę0×äµÓ?¥pƓodC?åÁ¢›h?¯ãþéÐí•?Äc¬­©Ü?¥äYbۍ©?¦@@êÙþ©?˜<Ԃ(õ?ì›Ë'Ù9?ªßdx€?°ƒsÉ8‡?¢Òîšÿÿ4FGL J1306.8-4035¿Ëi¨ê5@6-gý?[`À9wòŽþ5%À;ܱ?¨Œ|@­•£•ÆÑ@ìgßã*?µÉɍ'Ei?Ãð˜Ä\Ð@¯Ê]†ÃÔ@ZMxß?ï÷¡!MW¢¿á‰Óˆ¨°Ž¿ä{=ï홿ãX)Âq)8¿ïÿø]Ê5™?Ø®'úîôPSRpsr3FGL J1306.8-4031PSR J1306-4035?êŒ0^™«õ?¶bʸº»?­™å«ÔSH?¦ÛšYþý,?¼ÑŠ5Hvµ?±½WÚOá?æ6Η"Ôõ?È»Y>á,??Æôl‰ÃÉ?Ä•½¨©?À0¦5&èe?²À‡É?æÐuiŸûË?­XÍ°ÙN5?¼h4"cr ?¢Š¼ú}™?ƊÎW…?¤iRRæ_‰?æ»b鉲?ª]è…'VÆ?»ÏNÚå°?¢'GPñ?ǐÌìf]?§—&Ã!'y4FGL J1311.7-3430?ïoËgG@<,Š›ÏÔ¿À7…H-–;@À;fDH.lû@̓j5©@X²éÌ·Ô?˜¨yÜ9ý'?É!@ûBV@0 À~á@Ü4ÌesÍ¿›÷ý8`ªÌ¿ÚºìDâ2:¿âp·ù1¿ä²tË•¿ìËLd\ ë¿ëˆG◺FPSRPSR3FGL J1311.8-3430PSR J1311-3430?Ðßv*±2¸?',Íǵ?ÜÚ3ïð·?Ì×-\P®?ÒFUå^.?þ"‡±çS?À"&6<kÒ?ÏÖÔä-º?é?–äš?Ôb·?ÅWÐ?´ÝôfkŒ?Âàëü^?Ò¾ˆnÌÕ?³(}ZèŠ4?ß_½±£}?·*¬?›|?ËÃs¿Å[?®+'
ôq?]ÓÖS•¿›?V–	âË?íޚ@rO‰?¡,꓋j"?°"Þ£,¿? Ùšl—úÂ4FGL J1312.7+0050?éž‹6@Oœ1&éxÕÀ8ö6êÀ;øždÚu,@Öþ~ö€$@ŒÏkã}é?®>—?w9G?ßBÚ$ú
s@,mXê|àü@́±ñTA?æêZ±ý=®¿Ã)Ê(ؑQ¿ÚæÝR¿æAP—ÈB¿î釃 U¿ïû	h^ŽPSRPSR3FGL J1312.7+0051PSR J1312+0051?Zljsj?Zya½d—?ïÆb?Q:ñ?}x[a¹å³?výú¡ìØ?xV¦Ï§£?'Mf vK??°H™‹zN?î¬0'Õ/y?´c@"?˜,‰ãÅ}?¢s6ct˜?—-¾?¶
?"
ÞÐUñ?í2ÂêOçù?šA°ÞίÇ?°žy"?8?'júHŒ)?@;%'É—›?61Q…[J?ïNØP§~c?"±µÀÀ?•£¾yæú?"yA9!¾4FGL J1335.0-5656?á?ÝR@­µR\Ä&À9œVwÛÙ°À;ÞIWaç@``LpñÛ?þÊﲪâ—?¿ç¾€-â¼?ÚÓíNL"@^aIÆóo?ù;¬Îª?Ä|*ˆiÆm¿ãUeÂÒx¿ÖT¾\‡¿à£v'id¿í¼<e›:¿ïÿ¶Ï4†PSRpsr3FGL J1335.1-5655PSR J1335-5656?â9žÍƒ³?‡ÝÄ&PÊq?í¼­3Ÿ?±+0–#÷?³©Šã?®ÌÆN-£?ž¢N¢vï?£›Ñàø8¤?ä&ÎssÍÙ?ʅ•4áPå?ÕÈ:$.<á?Éd~5Í!4?¯\ôí£?˜KW]C?èü¼'š?¯YEB8ù?ÄGx¾&TÑ?¨h—Cᆎ?¹¬»¹û`?"yþ•w?Þe¯O¿i?´Y¡
Ò?ÛU%R?³é¤ÚÄ`4FGL J1341.7-6216?ä¯Þ€˜ ?—F~ŽŠÀ8><ÓG:À:$ƒÁÁ@y'w¾'˜@»ÒÄ]''?¿®áÕGšž?½ðÍÝîÞ@'Dé>?ÿŒü?O?ïl™Pž~¿à¼ÃÕ­F¿æsY>	Ðä¿æ0šö奿蛪ëÑtÒ¿ãä"ŸR¹PSRPSRPSR J1341-6220?ŒÀnà'?•.ÑÔD7n?"ñèbóìx?™@…¼??îlÎäé—?¤(
"»øë?žÛQí0Š? rÕa¿-?¤Å¬Tµâý?£‰z6G¡»?í¼É0%8L?ª³m24?´ñŸË Øë?—èqK¨™?±ZAÜP'Î?–Ì-†ÂY ?ë6ƒË҈?¡KKæpµ¡?'Ú~É:h?{»Ò"
'æ?®>ç÷Ô?ZÝ/ß?í…=ŸÒ8í?'Í"cC
Z4FGL J1350.6-6224¿ÒI½/Ã4¿ÔæÒâÀ7ÞÓMŽFÀ:™c²VÿÁ@[Ë ýQ@EE\*£B?±$Dÿa?ÚyJn¹?@%sçÑ5Z?ýoçáüú?îlT‡@с¿ÑÕ­+ª~¿Ý,iÀc¿ãÛJ^H	Ú¿íã}zV¿ïÿw¿1cPSRPSR3FGL J1350.4-6224PSR J1350-6225?OøÀw¾0[?EèÞ³Vwó?ïZ"Dÿ³?Ë´èu~"?"¯·ó¢%?]¨I˾x?n}ƒ"B?x"Ÿÿ,?êQ®}D?»æä[b?ÆB9ƒ…ä?»°*äq¼?^ŒïÒë?c$f383è?íM^kµ?"H8êìz?³rÀÒY/ó?"FO7•?$òÂñP?v¯.?êø1,ý?¥øsûæ:€?ÄþœÏ_{?¥õReŒ ¹4FGL J1356.9-6432¿Ûÿƒ£Ž"Àvò"º7À88É$¡ À:ÿ§Ÿì™ò@eÌ[7ß@?ÛÒú
x?±Ar'?Ö,?Ž‹Hž@çE™›@m¬¯Ëà?Ò àdõ"¿Ù¿v"2á¿ç>	…º¿"¿í*†Pçy ¿ìϦ›àœ¿ßŒ"2T;PSRPSR3FGL J1356.6-6428PSR J1357-6429?‡S
Äm;›?€•Ck8?éXŸ0ü?¾ÅaºŒ–?É(R'u;Ô?½]D¡»?˜'1*Œø3?¢º"…1b+?æ,e1Œžj?ÉÑZEUˆ9?Ò"Š=ó©?ÈJ€¹àÀí?¸¡-ßýÃó?£6"ûW?äNcUߪ²?´YÞkíêó?Ñ:íÜA9 ?°;|àG~'?'Âáâ(r
?i{³žäs¦?çEU3†û?®)ZÖ×;Ï?Ðß>ŠÅ®y?­¨0/³{Ð4FGL J1400.6-1432?îôÚ`;݄@FˆÚãæÄÆÀ9ɽaõ¾^À<Jã´oÞµ@"{±|9?þèm!kŠ"?»R´¾õ.ý?ÛRËêN½Ó@üC}-RI@zßæ¯÷Õ?¸µÓ9£¿¥TºÂ^3è¿ÙJT¢nªX¿çŠ×^÷\¿ïÿôa¼2¡¿áÎ"7blÝPSRPSR3FGL J1400.5-1437PSR J1400-1431?·Z¯~¥­—?´d¢¬ÏìÓ?ì5ŠÓ€'?¸üfÛ3?ŸŽªù9ƒ?®¸k¹<?µ…O'(-?³wŸ*`?êÃ*±Ïf?¼È²A`ô¬?´a_ˆIr¦?°Ë#xâ?¨ê5;È\ñ?–@PÐÃ(?ëó(rÅÕ?¤«€È$«#?º«L…¢ä?Ÿ<}Whx•?Ì·	&z'-?®`±>O%?ãÌÃ|0q?µ&9eÇ#?Äã˔¬?¥×
¶hÑ4FGL J1402.7+1306¿ÅŒÖ+ŠK@Q
Ž`€sXÀ;/´yï°'À=Ag2>@­@Ù0«ï\š@¸/ÿ¢/?Ïn"3¤?ïÿÓT¦J'@j†!퐒@¬ô•=¿¿ïÿÿ>¹ú?ïÿú÷''ý?wäò"䣿çVØ߬޿ïÿüÚ±'Þ?ïÿh@S§PSRpsr3FGL J1403.1+1304PSR J1402+13?Ùxá<?Ñ]‡›ÈO?â-ϕaÏ?ÑõC6ÿ?¡bï¦Àô?±4¾Øn[¹?Ár†¹2~ä?ÈBr)'b?énׂüÿà?Ë6ô™¿?±¤6u³8?­ÄèԈLÚ?Õ!"´õùÈ?°ÜJcU
f?á¼Qš8‡?±ˆg¸M?½›BŸVT§? ÅâÉÐõ?ÈEL(Š Ý?´ãӃ«?é¦"p3æ?¶!VÑ«.?›ÀÚm¤|`?'úÚ#uP4FGL J1411.5-6133¿Ð­™\÷Ž¿Ãƒ'ÓÀ8Žìø¼>àÀ:ZD4"@êýsޟ@1µ"±«?ʔk¿ù?×¥l`¦]ø@"Åyò4e?ô³[,°ã?é­Mî\ê¿ëPƒÀê@{¿å˜fÙS¿ç…NSJ)ð¿ïÿÑ;ÇVk¿åwÜ{~PSRPSR3FGL J1409.7-6132PSR J1410-6132?½5˜Lè?ÃéDià2?ÇMҌ›ÈŒ?Ä­°ÅíQM?æ…êéÏ}à?Ëí•0{ƒ"?šלÑÓ?"žT¹˜`i?½\Lt•}?»®ŒY `ã?ëßlú?»w©èè5v?µb;M2¾Ó?›½_Xo?ÇåÅü?in?¨n–f˜Ï?çZGIÍÊ?¬^íÛ`W$?F{Ñj!?4¤h(…N?É¡q@Îà!?°$Â͏E?é'»†D]?°%½Ós4FGL J1413.5-6205¿ÊÍÝΧÃS¿çx;»²À6hz™#RÀ:lÞO¬@tðo"7…@ªWÂ^´Á?—ZâàƐ?Ö:[4GZ@9cœ¥½"K?õø‹Âku?ïêF$§5¿Ä:òÚ¨'–¿ÞK9º5ñ¿ã|¯ŒwG¿ëқ
7 (¿îÑ݉¦PSRPSR3FGL J1413.4-6205PSR J1413-6205?CÖùÕVy?@⚝Àê«?í°4á -/?±ð®Ob¾?²XE
ëÍ?±Ûzûu?`"¢Îl õ?oÙ>mU	?î¹j˜Ø‹?¯õæšðb?­ò?)‹­/?¯œÛr…?@ƒŒÀ‹*?o$¾SØ$?ìQ[¾ü?£m蘕i?»i<ƒ?¢gîSÚ>l˜SÊa}>wêï"OÛ?ï
l‰^Vç?'¯4®ø;?žRkQ'¸?'¯2"j4FGL J1417.6-4403?ŽWcŽü¤Ú@0!æW¸MºÀ9~VG4À;õÐÕp	}@õèä°nG@wCõ"V?·Â<Pg?ÐÒpû•¸@%/ ×{|?üy/ï[íç?ìÃãNïQ\¿ÛÉ#…–,¿áíp¡'Øa¿â"Ànš'¿îà@$Ï¿ïýØ]y­ÁPSRpsr3FGL J1417.5-4402PSR J1417-4402?¸à{.¯?«Ò9=ƒìt?㨞k›H?ÄÞ×[‹à?ÒvÝd`ýÃ?œ+qúè?³'§û¸=.?²7.¯ïÈñ?é`|bqˆf?ì黦Š¶?À¼ºx]¿Ð?¾m5×Xå?Ç5Òc?¯bðÕûÚ?㔬C'3º?³išŠ«ü_?Êw|t«`?§p_'@?Ʀ˜Œ?µ}? ¦ÄŸZ(?à&ñ'f?³ðÓs–—?Ԅgyý v?°=¤"FQ4FGL J1418.7-6057?å¢#tƒ?À½ªÛ`cmÀ5÷'7ËHhÀ8¾èyÑ@ 
'e¾—@Ât֐›?uHऽ\?Ö]þÛß@6åÖZHŒ?÷¥óýhK?ÒJ»¿à€£ßÓ¿ÒRHù꽿åB
 À>õ¿í]+TB¿ïÿý`éNäPSRPSR3FGL J1418.6-6058PSR J1418-6058?ÂN'®Õ(?Ò/Ñ5äî?è,)ï2Qé?Òӈïݍ2?¹ aÆj?Âl#Ä$|?c?2mÛZ?s¤ô0$I?낰±ß¬Ø?Ä%gs†4p?Á¨@nÉß;?ā¨Fv?Œè¸5¿
s?†;Ë×K<?èóM}ëw?²4P†Ž[?Êd>"ö1'?±É|ZÅ>Yîž{Lø>fã1W€½Â?ëU«|»§e?³è÷o*÷@?©QÙ4%q?³è÷4¶7É4FGL J1420.0-6048?éÜט$F?͈y¡+´9À6­ûmÊÀ8·#24/²@ )Ve'V@üÉï£?³:à?Šj?Ô
›p3o@'^Ÿð˯–@`C¢?Ý?ï©¡ue¿æýôµÖ¿áSS.{=Ž¿æú˜'Bdÿ¿ìC[ªÌ¿ïÿöùŠpPSRPSR3FGL J1420.0-6048PSR J1420-6048?Ì]AÄGɅ?ÔÿÕ;µ—\?ÙdÒ/¨•?Ò5̉Á/?ØlŒî3†3?ѨTkZ²s?y%9üPc%?Ðû"ÞA?àw€Ü?ÑèÌ]	ri?Þ¬i_:?ÑÒÛí:'? þžâ"V?"ö›ü7?ãvèÙ?ø6?·Kö´ep?ÖòZŠÃ¿?¶ãÀäðå?xٛŸêµ>üÖy¬ ü ?ÃN{:{
?°zº£×ø°?ë,Nr½?°zìšSCX4FGL J1422.5-6137?éÜùÞ'èý¿äº'J9À7¡77¤²À;
Pø@@ €iڏ-/@Þý'¬?¦¤§tù|?áØì`@2£ôDàÚ¡@l
%É?ë´‹g\?ïӍæÝð¿ÉdxÞ°¿ÚS'Yáæ¿ë‹%nú¿ïÿCý…Ò<PSRPSR3FGL J1422.4-6137PSR J1422-6138?2I
$|?;ìoTª!?ïëB${€?m™$ïø+æ?btº?î=?kh£t¥?il°rtw?xãÆÙ\€?í.þ\Cµ?³À±y9æƒ?µÄŠ‰Š>¡?³TiB­ÍV?›øâ›í€?'mÙ´YÑ?êÑ ÅGïf?®–Æuõ¥?ÁX]Όĵ?«¥@1ý·]>ÄOS¤ÑÉ>ő"ó,I?ïǚôéä9?t²šÙ`@‰?|/û «Žâ?t±ÿÆ!Íñ4FGL J1429.9-5911?Üä%¸«?ôÜfŒ
ÀÀ6äh8éÀ:'u>p~@£3K[ô@Þ~pHg?˜Öoý'»ö?Ò¦¸¦¥@2PwxÝap@hš6Íq?ÎÐ
YË"¿ØÞ$þÜ¿äOC¿ç£ˆXÿ¿í½ªOÊB¯¿ì¯ÑêBÿYPSRPSR3FGL J1429.8-5910PSR J1429-5911?Q"A?ö£?U«2â?î¥cJ;Î?«œ©´ Å?¥"ÇÁ\'€?«ú¸¶—?pBùk(a?z ç}?êFCä3Û?Âu™æ?Æf¾Wh?R?Â[UVst?ŽæUÖsO?~̟'Ë2	?ë§×ýÃ?§ ¨cÂñy?¾ä,'[?¥\¬OeÅN>åÑIzcÔ>á½Þ¦&&?''A?""ý^€ý?¥ƒ€sH+9?"""#õRÈ4FGL J1431.4-4711?íbS×:'@(§¥	9d¦À9È9¼º0À;ã¥{O+·@x1ü@òR}{Uâ?Àª}—…m=?Ê®ÿ…Ö@%¼Cè@³æ¥;
¿ÙãEó¿Ý)´.pV¿éI-``gõ¿çH~ôÒ¥T¿êˆOúꊿÁë;¢ÃcíPSRPSRPSR J1431-4715?é7ZNÐ(?¸WvuÚ?²dªIçæ­?©`ò½$d?ÁðA¢°Ì?³<¦ÏŒ"?ëᄤzÍ	?¼–rN? vfuŒj?§£?¡_"R?¸ðŸ¨îю?¶/3ÿ<žu?åÿ Q84?®ü{|÷Š?¸˜~=¶ó?¢ñ1@«yi?Ë·?œÏ¥«?§t÷F ¬?êLü=e5?¡_V
¤Å?¬apÛ>s?'jÿÖ¾Î?¿gfÀu•›?›~.~	Ó4FGL J1440.2-5505¿å¿ºž)ª@%4¢žûÙÀ9ì"ì"qÀ;b–ãܳË@´"gÑK@óìÌG?àåîqbBë?Üdrûö*@?,0	³@"K>—ÀQ?ïdG!ý€Ê¿çK;gµÿ¿êLL¿vM¿í¹Ò9?Ö¹õ͔ô¿ïÿþó…õPSRpsrPSR J1439-5501?è$šÏа-?ÄÈþ
[-?¶2вÑð?¹¤â[H?ÄT,gTQ?À¿'îåî?Ûôôp`•W?̸ÌÕU³?¥¥²óúö?·ÝŠ`ÉÕÃ?à«*˜E?Ê¿¤E"?ÙuG9dÕÚ?°‹L¦€×{?Á²XαQ?¦LêâT't?Ýü_š3Ñ|?±Mô(ºm?áhüZض?À³RxÕ,?soÿ—WÆ?{ƒÔó¤êÞ?ÜፊP5‡?À¿9ä4c´4FGL J1446.6-4701¿Þ%ü­©á@&×W÷7ÚbÀ9¶Ë¢*aÓÀ< #‹öC@úÚý8?ÿq'Ñ8?º'pÉÂ?ۏç¿€Ë@L÷‡‹z@™·
ó³–?ï÷ €=¨¿ãœÀ€
V€¿Ú¢J"
¿å1&s1P¿íˆ}ˆkI¿ïæ¡à×PSRPSR3FGL J1446.6-4701PSR J1446-4701?†WËÉyé? HÏ?íøhpÔ\»?«F'ÝùJ?ªã†[ìg?©6@›òÒ?¢ñ`´™Iè?¨~ÞÚ´}?êxãÀê"?Âp1iö±?Á`Ï1Hý?ÀxΔŽ˜?©X¶]OÅ-?–Øc)!r­?ê?põÖÉ?§¡W7y®Ç?À­t¤Ô³?£D^%C½_?³©E$ˆ:?ãQ™r>9?ãcð‹œ?°#+­bÁ'?ԝï¹?¬ðT‰ c4FGL J1459.5-6053¿ê­q™0¤I¿üªØ>À6ÎÿÄpݹÀ:p™ÆC@›h,**@ՙÅ8ƒÕ?–ÝB÷݂ä?ÑsUAûÍì@3fÖE"@«"Ï€0g?ïÇ€\±²¿Ü ïCš3¿ä_Eà´á¿ç—×øyùÁ¿îVÁ"¸Ó¿ðPSRPSR3FGL J1459.4-6053PSR J1459-6053?q©
\dU§?ˆÓæpoӛ?;NÖ?«g?Äà?£?ÿ'Çà?©h•B9£?q@þþî?}|VóT?ìŒß÷ÝÈ_?¹M¸¢>W?º"ð`½?¸Ü´:^Å?¤!æñáøv?"ó;×+ù?è
P<º?±&|ù!?ʧjFŽý?®<^Ð%>ҁÃr8ô´>ќ+Íeóg?îï« ?EŸœÝr?¡Q@@?D{¸¿g4FGL J1509.4-5850?ì"Ó±~¤¿ã¶¡²lÏ6À6áÐË_ƒÀ:,…'¤Ø'@MÒ±=OA@$³"כ]?žœÁ}t† ?Ø¿Ì^<÷,@3¿â`²È?@¸l"}Ðæ?îrjJ÷u?ёÖ¤¿ÝìWڎ¿ä‰Øá®a¿íW®rn²e¿ïÿÑ ïcÑPSRPSR3FGL J1509.4-5850PSR J1509-5850?Y…Ó|¡¦Æ?[üt™Ø\?îN}Òl?©¯ƒÎêú]?ªK÷†ô2Ë?© &, ä?mÍ°‹o?}mŠ7L	?ìš^=?¶oÆڏFª?ºA7Š¹¾š?¶`J±?…%‹1{v?}ª0Eç`]?ì5áE-
?¦Î‡"²?»²·´¨A?¦ʁXºô>ã'e
ÜùÖ>âK¹þ'«0?íÕŸÌO?š–¨ùë$?±V¡Æw––?š–öÓu|4FGL J1513.4-2549?ìïVv@:ö—Oß;À9±WVO˜À<DC;¾òï@ç笳@ÃÝ:ZM?¶ÿ‡_/es?۝}ÿµ,@³Ñà2_@6ˆ*?î˜?ËG¿É£u{S¿àBuüŸ|¿èÊXÿ°J¿êþÈs¡¸¿ïûý<aOPSRPSR3FGL J1513.4-2549PSR J1513-2550?'Zõ—§Ô?
ș'Úó?îõɤ‡@¨?™þ³Àô?×«®à-¼?‰`?'vÆÉ? ø½a|#? 2ˆ
?í€dŽ~¬t?®]V?¾î?§Ù¾Z³¼?¤À9b×ã?³VŽ^êÝ?¡˜óð?ésŠxõw?­+'¢˜ï,?À†ŽÛz®ˆ?£Ç># Q?«œ¹'?¨"½ÚÙD?ëvð.Lêà?¤µGƒ¿ó?¶Àõ‡ÊL<?¡ü¦ÂCL44FGL J1514.3-4946?·™·@ôfð@<½±¦×À7ëýŽ5¸IÀ;t]ýâŽ@"ÜÅ×?ý;v­‡?¡UÑÿͼG?֖!_K?@1,M‡rO©?ûiùée‰È¿ßNa6ü–¿É‹¶ÂtYC¿Öå+ž{޿ߜjÄÄ낿ìë€K꺿ìÙä!þ£PSRPSR3FGL J1514.2-4947PSR J1514-4946?rê ; ú?sÝæ7–²Ê?í˜Ø<Lˆ?°±"DUÀG?²
œ‹Œ$?¯™Úí‹$*?€÷)Ý#?"‹°O{?ìɉ=
Æ?À¿-cð´?·"Ñò»ím?À7QQÊ«?øïÈ؁?†»(O½?ì΢@".?YËô³­?µ‹ÐӅ?™úLàŸ?(8§`C¯?"üÖõ?î@¦€
?–ëê>Ý6?®ƞ7»·?–â¢04FGL J1521.9-5735¿—L¶^s¿ÚZyMBÔÀ7N#'¬?À:ƒùd@ŸĈ/º@ûbó?£Ó›s
"¼?ÛzA—b@/I¯:ÎÄ?ú0«?ïҟà·ö¿Ñnñ$oöÞ¿â'†ø­%¿èç/N¢¿íázn['n¿ïûÓ {‹PSRPSR3FGL J1521.9-5736PSR J1522-5735?U™.Y]!?YÜy²ÄYè?ïK¦"F…?íTÜD¤Ã?•;"$IÉv?œäÖXœ4¥?nÝÑó?…S/¤p(?ì¯qÑ~)?´ {z@?¹Š¸µ?³Ëát14?ƒò1 ê?n–Neû?í[¨éš?˜UsðV×?µ,Dy²š?–…µ&=ë+>Úk$<ê׫>Ñßß:ˆ?îé#1¹žG?eÓQl.*?¡lù‹D4J?e>]gôî4FGL J1528.4-5838¿ÃÓUÊYLo¿ü\¼™yÀ8Î.«6$À;›mµæz@ ¼Êv0^@(éÛÑLŽ?¸Ö—Péý_?äi›Ô×]@#»úëÄ?ÿ#á?¿të…tž?ïIšé$ò(¿Ômc°©€—¿äÀ|A™þC¿í蜁U€¿ïúÖàÌÞëPSRPSR3FGL J1528.3-5836PSR J1528-5838?RoÖ¾
]?N×Ӕ!âŒ?ïbÅëKè?"œ…É+Y6?'€Jy|?"%(zÛ?vØ?€}5(šéÕ?ëMPö&¸p?»/Ò­jß?ÂÝftm?º÷=µä"È?…¿¨Ñ?w'•]Åè?ìÓá$…?ýL±¥Y±?¸Viq¦º?›*º¶Zå?Elõ¬Äå?1Ï£×ÑD?ï¥v:?‰ÊzDÒ?¿éŽÿ¥?‰–¼j*Ÿ4FGL J1531.5-5612¿îw…ï²nÁ¿6pÇ¡À]ÁÀ8žo¿«À:‹Á#K^£@")K'ñŒ@E\{+‰?À܃ä{•"?âßøãú@×P +"@½(ûL¿ïûü€¿?ïÿþBe«+¿â@`xÜ¿éÚÔ,<ží¿í…H©¼ýL¿ïÿþBe«+PSRPSRPSR J1531-5610?'?cÜÐ?•ÆcZí¥?îr‡¢n_?§¨ó–z¿ò?Ÿo¨£²WS?¡Ñ¯êÓVQ?…«@DB1N?‹ÿœèÒ(É?áٛÝ~Š,?Ês	Øqõ?۟nBàÚ?ÊÝk'4[? '!)ö?‹ÖÜ=Ù§?攤ÁI?µH'Ö?ÐÄsµ¸/6?³§›*4?hóV(s©J?T5bïÝ®?ãnöޘ@?µ±J«[̨?Øð+–~˜ˆ?µ–ПâÚÕ4FGL J1536.4-4948?¸ÅN¯3¶p@%‡CUÀ&À7D¾'wfiÀ;i
	Ó¾@4è-?þXAZ=c8?™t-EÕĐ?Ï¥}'þ®@48ð"aùð@+SÔhx?ïø$B`M¿ÎÒ&þÇp¿ÝÔÜeÇ¿ààÁKdW¿ê7Pþ¿ï-¨§b°PSRPSR3FGL J1536.3-4949PSR J1536-49?Žf"œ[:=?~"Ý%|?éŒ}ô–&?ÅW}ÙQ·?Çét¾góÆ?ļ9¼9í?'"ÑX¥ý?"íV0ð=0?ꦺ™M·7?ɓàÇ÷
%?Äit>]ñ?ÈÖ¾'Û}?¾šÌP9mÁ?¦¿œ<Zu ?á€ËÇólå?¸#¤¼¸i‰?ÕWµ\
ÊÆ?µ7r€Õ-"?¿îCZ4?ãpÇkDé?î2rO©
¯?›d¼‹}¶;?¬ÏûoQ?›_㠟q4FGL J1543.6-5148?×5±¹\=Õ@ù#zX‹²À8À/#ÙùÜÀ;3òuÓÂ@wP»¯C$@C‹«`k?¸ÓfC«Ñ?ÕY:Ë@7Tm?ž|@
jØf¿ãuIX8¦?ï³±=$M½¿ã˜Æ5¿åÃG
H¾¿ïP²4›@¿ïþ)ÉßPSRPSR3FGL J1542.9-5141PSR J1543-5149?ƒ&+'aVß?–ûÙ{H?ï'Z?šUüç…@ÿ?'¨(íñÂ?"$ƒå$¼ì?—Àg?¦¹çå7Ãt?æ©_|:Î9?Í&<^Lz?Ñ<Eƒ+?ËÛLd-£·?‹¦9ç?Š&Þç
þ?éÐæc¼¦–?­œ#s§?Å
ñ¯¦D?©ðœ[Õg?—Ý/|é?}åÐ.î•?èVdÏIJ—?°3tÿöþ?˪Æß'&?®-y ɹj4FGL J1544.0+4939¿é:6ûMa@Izd×ñÀ:ii˜JAÀ<»´Ci@V3Á£xë@üÂ]Þ?¸Œk2ÓçÉ?ÉBÔ+'@ï|i+?ø
ˆ?ü?ë08AíH¿Ë|ÊÌ¿á"lhÞæ«¿ã_j^B«v¿èÈX>/'¿ïY§ÜR{ÎPSRPSR3FGL J1544.0+4938PSR J1544+4937?æA`,3N?¿Ãv"¿Ò?¹m†íh{?°œô	€?ÊCñ½
Š?¹áûˆñåN?á½kžÆ#?ɜռ¿?Ð։VIá¯?ÈZ"o5?Ç]@ðñ$?¹ï4÷²¹?êwöŽeß?§	™íŠ?°Wo´«Ñ?›ÀF¯&`S?»èÜx[F?Œ-Qc*?á…½ßúØ?¯á?Õ>??Õ̅ ô4ñ?±LN@á"Ì?¿Ù½/Ux?šëډК@4FGL J1553.1+5438¿æ§ËÉËJ@G•ˆ†aÀ:—ù_ÒÎoÀ<Ìò8— C@¼<Vžó?ÿhfx?¾í‡¾‹ý‹?Òó†ŸìÄå@ïÒ¦*¡"?úݹv®³?ハŸ€¹N¿ÑMÓؿރ{Óö¿àïgAÒé¿îgÝÿú÷ƒ¿ïòO]‹KxPSRPSR3FGL J1553.1+5437PSR J1552+5437?ÜÝï‰S?ď'8¬s?×iŽ¢X™?Æ$Ò¨®Å'?É&Ü=Î&?¼W™¨¤?юA¯Åì?Æ2koÿ°å?â(%ǸÉG?Ë>®ç *a?ÄCP]½O?¹YóqšÄH?ØïØÏðå?·…lü	+5?Ü|‹fŸ<î?¸lnJë2›?Æù	!¤^?£ÈÖ:‹J?×]=m·‡?°U¼^'4ù?ߐ'4o«?´ld?Â$chõ±?¡
9w4FGL J1555.7-2908?݃®	W@2€‰ÁµA–À9°^©Ã)À<y)·‰o@¾€+ßVè@x¶Ë?ºˆá~<ò?Ï)U–µd@
\¶â¼y@X=®·8?Õ;Ä|FM¿Ý¢ˆá:˜¿é	ß|Ò¹¿é!YKË°m¿èÒUºc¿ïÿ¨âaßnPSRPSRPSR J1555-2908?ã{:aj?ÂQB®ф?Ïgu>­Å?Àº6^.Ø?¬.O̓?´UÈDmž?Þ¥:Bô?Êc€ea7?Ö¦½·M€?Êdj"ÕÜ?Åh"Q|ö?º"æ8'÷?åD¤6·?±¡Qې+?Áü¾ÏëR?§up1<=?É­<ܟ9Ò?§în‡1?âæ_ïŸ?¦>SwÜõ-?е|Júˆê?¨Ñby"Ø?Æo‹/³?ÐœDÐg4FGL J1600.9-3054?µZ0LHäè@0o‡z³$…À9¡çÒ␃À<lU\Rç.@!›_íP{?ÿd1m`U«?´£×àýz?ßü©ß7©@"ëØYÈÉ2@Ëuå	"Ž?ï´~÷¬Ê¿´FÕQ€¦.¿ÁÚâ9Eœ¿ÝUÈbÿ¿í]v¾"e¿æßnàˆktPSRPSR3FGL J1600.8-3053PSR J1600-3053?œmcxæ?z˜à¢¥ ?ï€Ӓ·¿?yÁíò"?|·»o²Sñ?"ئgZ9?‹%p¤ùõ?=ƒz(ƒ&?íÊð0¤T?µwºÀ@?¬–düŒ|F?´2±T
r?¦Í-f½cR?˜c	‡+ÌØ?ì"Ê+ƒ"(?¢n"zF~?³ƒð"µ?–¸g½0…s?ˆ«ûӗÙ?s->4‡C?í÷xV'ã?—/H^'?ª]šê›Ð?•p[%å—O4FGL J1614.1-5047?æf­œc?ǵ|N/7üÀ8ãpOô4À:2ðXõ@ ,3¦¹Ú@IèÄzô?ÊÁPlÕ?Ò(}ˆÁÛ@	²|¤–LÞ@:–ê<Ê6¿ï(å!,u?àכ³¿åWiþ÷Ak¿ä(àwúc¿ïÿðÇô ?ïýçAB?–PSRPSR0FGL J1615.6-5049PSR J1614-50480?ÀA2w`:?¹Oû<»S?À=÷~ºÙ?ž9ò?çà:ÓÞy;?ƞگ'ãÙ?«ÆEÙ¶…¹?±+'PJz?ÀX°
d½?òhQ?ê<Åva>u?ÄçFF_?ÀP}5˜¶?¢WO!ëÏü?ÅÓò1£Œ?¦;çÿ׸?ævä&RUï?«©!‰æD­?]Á©Ë²?Š8oRÖn?±à«†ä? ˜Ú€â·?ìãô%@Æ?¢†Ïf'4FGL J1614.5-2230?æ䧜¼Ž¼@43Ä~I±ûÀ8fé†.ƒÀ;àş±á@ê×™"v?ý™'Í_š?©u}äI?ãMˆÿ˜|
@4f^‰"S?ûq…Þz?ï
–1ÿ?ëP6®è¶7¿Ä9h6¿ãªDâˆõ¿íCçì
õ¿ïÔ»¾²'ÊPSRPSR3FGL J1614.5-2231PSR J1614-2230?F‰ss6ÍÙ?IdÃN"tg?ïìôœ\yâ?f^ÒW¬+J?ZÒ
pÔ?b˒^—³P?y\ë¿ú?˜yÖêuè\?î¤áBA_@?´ã¦$…`?¢†iމÔ?³"	+½¡e?Œ½$À—€?|&
{í?íxI­ãµi?"P~χ¯?°ºìJAÃ?'ÛÊ2G>Ñ°õÒ£n>҆Ñfp?ïàæPˆw?a6×ü¯oœ?oÖüúþ?a4b+`Y4FGL J1615.3-5136?Õ¨ü|׆¿á>Ó°ÜáÀ8Ýñ¸> À:ˆ™|=h@@ *¿;>Åc@¢¡<ü	Ñ?µ°@¥½£?æDí¥Šh¤@&Xn\Ôí-@´€?ï gžÊ°é¿Ô†.B]•¿ÜÜ¥‡äep¿Þ$ò¾#Ñ¿í²
©§-׿ïþÊô<'PSRPSR2FGL J1615.2-5138PSR J1615-5137?FkX&Ì?F=[/¤D&?ï8-ù±ŸÐ?¨|¬"ñ)"?˜IÝoÜ¥?¨UhXfX?qØYÛµÀ?|£YÈ®Î?êªÊµØý?»ÑËvÆ*?ÄÆY¾[½?»•gPûƒ?ˆî9Ô˜?yðÌ̄
?ìV>­Mû?ŸVBUwñ±?º0C[
0?ždÍö?Û²_»ò?¡¨xAj?ë¡(Þ`ؗ?¯½ÁÓÚ::?ÁxÁ,q¡?¯ºMŽ¢ûŽ4FGL J1618.7-4633c¿ìÓ'"Ü…@•ê˜+ÛÀ9=#I±À:©ï§Ã(@p{¥<åä@$º¼)?ÛwNëö]À?×» ¿þˆ1@±+ÿbKO?÷°à]"p?á'‡|a¿â8— B•§¿â[eŠ¿a¿ç™è^x±B¿êg‹"ôk¿×$*í"1PSRpsr2FGL J1619.0-4650PSR J1618-4623*?ź
XmPò?¼á·>0{?׈á®yLK?˼'wy¥m?ݚ¥P>?ÌJ¹(í†?·ì"µ(TS?¸‹"н#Ò?ÃÝ
;_™?Æ%蒾I?è8Zƒ1?ÆA¤#6ü‹?Ãq"Ðd'¥? z?}|
w?Äuß~‹Q?¦žÃ§%˜!?æ"ìD!Ò?«lõaNX?~Dl/á×o?g¨þh#	?±eøš?H?¦iÛÍàJ?햸#¬ôf?¦‡À o¨4FGL J1620.7-4927?äP¶3á·s?ÙâûB+»À6ǎö¨hiÀ:hõ2F¤)@ K6r,@i9™m$? Í¤Ážy?áyß¿î˜@7©)þK?üÁ"À?ïK$£Mx¿Ù¨ââ¸Ç¿ÔÔg ÎN¿ÞØ<'g±¿ì>ß¿Ød¿ïº–ÔÃ;TPSRPSR3FGL J1620.8-4928PSR J1620-4927? Nr®ÉN?%&$ðTj1?ïË&¸«:H?†‡,Ñx?yê2öÍf?†D8ixß?cq´€ Ø?qJ×ÍZÊÂ?íPà|»\g?³$J¾šxW?´Ýnv$÷Â?²õ"3´z®?€¥ì†?s¤×—›Þ?í"…¤>­Â?œé;koF?´×2*Mµ?›4Kíô¶>l°)9†l>v\qϸƒ?ï²µg,Íy?zí±à©v?ƒRŸÂSÅ?zí¯†)«4FGL J1623.0-5004?èMÕmk¿Ò©÷þ½áÀ7…J¼Ì¥À:†Œ"ÎX¾@ –üªàéº@Äہ›v?«öÍ&cìä?Ù±y_<{†@%¶å«ÀãŠ@;ùUkí¿ï'½ÂmÎ:?ï|µ«¬¿Ðÿ3ý2›3¿à«;³´M¿éú¿žæàt¿ì^|PSRPSR3FGL J1622.9-5004PSR J1623-5005?bbÂ3Ԃ¾?di…ï—?îÐ$»­?¨?")¿à~?¡ÙS*vý?§aŖ¾;I?|¹{Kü–?ŽŽh0¢Å?çA)Î8o?Ëjåà""?Ñ
ÆwAò
?Êõ-¢[ûÜ?¡#—«û?'8×¢ŽÒ?å'>'.Í?µ³ËȓV¢?ÒÚü¬æ?´–%:ææL?5*¤—QN7?&Œƒ*….Q?ì™,ZXޑ?¦èÏv,k{?»!rˆ¡º%?¦á€î9¨4FGL J1623.0-0315¿Ò256ˆ@>«ÅXdE$À9'˜(€QÊÀ<&‹ÿ}#A@IèVk@3/‡­?³xýlÒ¼%?΅÷eҗ½@@,Meä`@±©'×	'?ïô"'òÜ+¿Ýa=@'¿à)Tݧæc¿â\ä¥5¯¿îvSCsó¿ïÿßÿY'íPSRPSR3FGL J1622.9-0312PSR J1622-0315?Å¢•~â%?ºôúýè™x?ç\,è=£Ñ?ÁŽž¬^G?¹ÙmÀN×2?¯ZÚJ~ÿ0?¼azù\?¸_Ò]Å>r?é¥]'?ÀëŠÉA¦1?¶ÅF"õ?°ÇÉחü?Õ/©*80à?³Ë½×äË°?߉é•C¬¿?µ´À…†E?ƌځDÀ?¤‹×º<I?ÆÌtŒ±à?£3ÿóö—?äˆpZ?¯ã06Ÿ'?Ç5×?9Œ·?£N€ÿª4FGL J1624.1-4042?Óð»ª÷¡@©¡N™ÁÀ8P
ýÅÀ;fe€…@w?<ÖÊý@z¼¼´PÕ?©$'bq÷?Û¢‹EC0@)ؽ©CZÉ@8<­…v?ïúeA"_%¿Ñ,}a¡Ì¿à
¯	mg¿æ'"|ú&¢¿ï	OŸz"+¿ïî?CîKPSRPSR3FGL J1624.2-4041PSR J1624-4041?g¡ÁNq?lOڍÍI?îÒ£ø$)T?£
ˆÒ¯_j?¡d&lÑUã?¡Ç"`–k?€_i-ξ?Ð´4rÇ?ì4Ðq_)?Áoþö|õ?¼MOLä?Àä(‹wþ?ŠÃ]	/!?|ûª*7Tç?ì‡by~Ý?Ÿç¨éZ5?¸l€–~$÷?œ¦ƒÆm??L¡uÒäà?.ÿÐh³Ôö?îm¸hm"a?'–²«3RÃ?¨åà6;$7?'ŒÐÊÿº4FGL J1624.3-3952¿Ô@˜»<|@ÃÝ}8ÐÀ9ž3ÆàÀ;ž6`å@'úÇ[ô@üGÿsF?À¾Ëê'Q?Öàþ]ª¨@vì["@æßóÈd?ïý†ì]Œ¿¼vјŽ¸¿Þ5úÀñ¿áË8Bf¬Ý¿ïÿ›‹â ò?ïÞEedÞ§PSRpsr3FGL J1624.2-3957PSR J1624-39?À×­wbÙF?³¶K'`sº?Õ+¼u\'?ÇGèÛ‡;?á46gyCå?Çi ,¹¼D?Â:É'îî?Â]"í¿?Ú«‰Tz£?ÍP˜Ÿ‹ÊG?Ü7ⴄe?˱ïýõ"?»-aã0ºë?¡vÔÕic?áÉ£ð9ó?µ.¢ø§?Õ¡_¦Á³_?±SÆf¹°?ÈÌ€LØê?§+àît™?МüêŠMk?³­ù>¦vM?á~ꧣ?¶r0±<7±4FGL J1625.1-0020?ξ$ކ³Ž@?Ö9.÷<À8žÎR
À<CN3iº@3ç}R;6?ý}›6QÌ?§™(c)"Â?áE"žæ_›@1â">iƒ?ýð´`Dc\?Ãa}Uì¿Ï§½^DÙÏ¿ÑÆmãv¿ãwlH'·¿ï¿¼¿ïùM^W¤,PSRPSR3FGL J1625.1-0021PSR J1625-0021?\²[Ø&Ù?oÔÛ	CÏ?ïÞÉQ÷€q?ƒµmXÓ?b݀l$?|1ëúå[?x¹&\'m÷?†ø$ˆõ™?ï|´—Kª?¥ôT0)'?–¢Õò/?¢µ‹a¥¡?‹¥næÃoë?y.î"Åë?í¸nd!¥?ÍY<¯?­¾m	ª?‰óžU-
?
LA:hÉ?ÑöN¹ñ%?ï ß†hçù?uv%êò?‡­Ò$‹™z?uk&iќ4FGL J1627.7+3219¿í,â჊†@EžNaŒâÒÀ:ePÏ%l¡À<»kõò`@1ONFßã?ú¬d\ êÇ?Æn¢ŸýŒ?äv‡*¯@Ì ~$É
?þô¿ÍŠâÈ¿å<ççÛF¿ÛЏ$Äì¿Dr}Ëݹ"¿äج¿f1ã¿ïÿÿ" 5•?ïÿ̾ßú&PSRpsr3FGL J1627.8+3217PSR J1627+3219?€Yô¤i?¿ÉQÁß<?és6Aša·?ē½Z¬^?®Ìn~‡Ræ?³E•«?°;K›Ø?±5â0©?떘¶ôw?»'+¿t7r?³îªÒ@j?±[¯o_]?½0œðg¹?¡°Y=:€?è
Ý!­?ªô¤YöŸ?ÁHó5?£Ë5mÎ̛?Óx'@ëLï?·9UÈ!'?Ü;ó
 Ğ?¾Ý7Òæ­§?ÐKŠ±óîs?´=8¾ýö4FGL J1628.1-3204¿Ó).º•@&ûžŒG¡À9>	 '²À<OB]r¢@ú=ºË˜@_'c3?´S~¾].•?ÞÏ·£Dé@!h0Â?«?ögR]šæ?ïôî<‰¿ÙÕRAì3š¿ÝÂž»¿è˜f~9@é¿îÍê¿&¿ïóêþ'PSRPSR3FGL J1628.0-3203PSR J1628-3205?lðGTAD?hN--ˆc?î"ö3Êf?¤X²AKӝ?¤çÊÎw?£{1K¯Ý?‡?ùäD?Ÿ
$›Ðy?í,r~)¿ö?¾
mRà–?³»uwÔ?¼+?dÔä?˜þ¾ÓP?ƒ6ÂÜÀ!.?ëV(]†'?¢ø'o#ò0?½ÅŸ3wè? ½–jWù¯?V7H\
?@vœ§]@ý?îšdIø?'‹>ç#?¥­{7ëM?'cû&ðÞ4FGL J1630.6+3734¿ëª	I@Ešgó
NÀ9ØScTc/À<OÓ7ë)@(¡Ê?©¹?þ"•üV'?¹5Rr=µ?åR›¾aúò@Ì­~«@Oú)ƒ\?ïĬ½bÌ~¿ÖN¾ÿږ9¿ÓÖ¢¤V§¿åˆs¡¸L¿ïÿ÷Ò4Û?ìDÇ_¥'PSRPSR3FGL J1630.2+3733PSR J1630+3734?'LðLù´?iæ9ÿ"?ï5£Uò=?"þ…;dæ"?ú'ÉÃzÆ?~i!-ü?–ô,u_?›
†8
RQ?îlÐôÄ¢?­–/mæs?¤¹£ö{$?¥‡y9csW? ¤zBçAc?PÑÉ`¡Z?ë燅«£?¢HenÜêŽ?¸q†¶/9?žG…®·W
?£¥{)4Ä?'†ÙÜ{¼(?ê|Ö©ŠZ?³Ø³º[Ô7?ÂÌ­Û	j?°ˆò·c"4FGL J1634.7+0235?ëOdÆlû@?T›«–òÀ;p>Ȓ«iÀ=8؆>s@I á÷×=?ÿîóhB¹?Ô¡…‹Å›€?ïüÌnØû¯@(™|=h?øš€Y¦‰?´/ȀÈùj?î$¡ÿ?×ÐÇãÙÙ¦¿æµ¹?§4ã¿ïÿý±q&´?ïÉ+ø¬N¨PSRpsrPSR J1634+02?×èY÷ªzü?Ê[¯~"ä8?á-γîƒá?ÌSê_cž?¶ð"áõ?³'¾	=\?¿<j°¦Ùþ?ÄÜ;ãGÖ?é¡Ûvb–Z?Êu&>øy?³´¹œDs3?°ÕØ3»CÓ?Ñ`‰'
;Æ?³ÞÍL¨Ô¥?áτ»@ò?µ™·™Ep‹?ÆÙðç¿ù?¦™â̖?ÀîícýŽ?°+×y0©'?ꀱy¯Yj?³œµ›2Ð?§',¯zs+?šîÎÌ4FGL J1640.1+2222¿ï'Ö!'Õc@C&³÷+EÀ:É[ÇÎ`À<©'¿9@æ!ƒˆ`6@Úmý3œå?ÆR6X¬"s?Ýd)uDP@úÃ")´@¾OhÈì¿¿ª›©ä@?ïóŠ¦·¿Õ­N ¿ã‡ÕÍÛ@¿ïþg¿Víx¿ã_Ř%%SPSRPSRPSR J1640+2224?ÆàÇrìŠ?º¿UÌÉ#?ép㷒ií?¼ôÝ] Ð?šÝMvRN?"Ơ΄?ÐÜkt¬?Å,ÑÛÛ?ãH$9¶±u?É&º*a ÷?Á'XB;â?³ÃµÀ8ü?ÇýÙl[¤?²9Ŷ>öž?åq‡•þòO?¶ô@]ÀÉÐ?Â<àΗÛ!?£Kh:•b?Ñ°ÇV?­Ý'/?â™2Œmcï?³ÅHåñ?Â:þ?ž4??¤«ÉÚÞ-S4FGL J1641.2+8049?çŽxÝÑÔ@?ij=¯øÀ:Ôcb¥ç†À=f{_ï@ªž+#Å,@O–ü0g§?Â;¶šM?Þj'Ûdj8@°4ß۝J?õ;qE< ?ì?i¢[?î§À&KC¿Ý¡<é?t¿è®JáO»ª¿é¨äÅçÖ>¿ïýªë&PSRPSR3FGL J1642.4+8045PSR J1641+8049?µlª¬¦¬?´PþP—^÷?ìÑÀÁ(?·('®Ö(Ð?*]7…@V?'Ž–|׫Ç?¬j³Jiê>?³CéPFôÄ?ìGc»ZÞº?½d¹%:l#?¯ÿè*"?­aG	?ÖVªq[?µ{Dӏò?Þ°¼žã¾¯?·PAC4y¦?ÅògmVwë?¤ßZ3"@[?¨¨»0çt?•wUÑy2³?íÛپņ?Ÿ•Ü=¹å ?"w±Å€J?ä~ڌ4FGL J1641.2-5317?ÈòïïÀ?\¯-•À8˳;+À;TÚÌiÐ~@=³é@åŸ+©Ò?³²¹¿î†Ë?Üe;µg@"n½	á*R?ÿn±†uO?ïîºþn/‰¿ÔDûb6¿â¦KÄ#°ß¿éKF¿Ä§¿ïýu@ô¼Ö?ïy§4ƒ?PSRPSR3FGL J1641.5-5319PSR J1641-5317?³|åŒÿC.?¬âŒŽ?âåÐw?ÊP¹o{º?ÕU&d¿A*?ÇÁ¨ü¥ë?š—œ'c?±»v8•£?çöӋWÔ?Æ¿Á"LAV?ÌÔ±à~?Ä?Io‹O?R]ô\ã?‹`–	M'C?ér½¨I?®ç Op›?Ɗ¾B÷³<?¬	~6bÃ?‡aÎ]æš?t‡>
»%½?ç+)¬_?´ñ¶Jµ]?Ðîž4áz
?´euªTü4FGL J1648.4-4611?林g%S!¿éÏ]Àû]YÀ7ÄfUŸnÆÀ:b¸[ü€@ 1)ÆMå@£¢Y[»è?°áà°.†{?Þ9ÚÙ)ý@$ê ¼8*@pjKM[?èY}êçj¿àÌö¡¿Ë¥ô[\6¿áڕwËéx¿ëbšÿË&Ú¿ëDLˊ­nPSRPSR3FGL J1648.3-4611PSR J1648-4611?qâ>»Uå?—›êIö?îþ{'É?¢…²ê
Ø?›¸neã?› $äú…Ë?xÙ¡þ\$2?KhwíF?èÓ¼"òû˜?Átç ÿ`?Ëê@œA0|?ÁU–uý"?œO¡kI{ê?ŽQNèŠT?éÐ	âóm?«ëïÛ»ú?Å5äFÊnÌ?©©ZÍú?A÷
\^§R?0šLOU‰?èúm¤ÃvJ?±‹Ú®õÖG?ÌRb•È2?±‡ç2
!4FGL J1649.8-3010?ï¾¾ì†ÈÔ@"lQ¹07ÖÀ9`òl™†NÀ;ë]"ðÅÐ@I í¶Q@§ºÄŒŒk?¹"ù¼o?ݞPõùl@ ™÷L¿éñ8ŸXËH?ï¢ý$ƒm¿ãÑàd)u¿ÚºûéðÊ¿ã@Bæ.ž¿ïÿþˆ0»Š¿ë·é íö¾PSRpsr3FGL J1649.6-3007PSR J1649-3012?µ+j&TìZ?»O{OÆ?ì;œZŒú?¾ù
"\²+?¡ïf
†‡
?¤˜¬7ù4?†K¹Y£ª?¬$¢"':?ꬩó6Áw?̧§ô*ÿ?Ãè¦g_ë?ËR†Y·?¯x¬|@ç?›ÊÉAsá¨?éao)úwý?©bB+§{?œR÷Ò?¤cêŠ?&Sù™F/?DoÔÄ_?îÇÅ0W8x?•Ú8¯†ý?£mYóm?•Î¥TÊñ§4FGL J1650.3-4600?ìÝÖº}¿î€ž@GmÓÀ7¬r•;fÀ:GÏASC@80Fé@bO̲+?²N×>ã'?ÞÁ»=j@&–V«Þ?¼@RÞ³T*Ð?ÜÇ<? |L?Ë¥ñÁ£ÎÒ¿à4äv]¿å½‹±yŠ0¿îø/¼†-¬¿éœŽ i¬íPSRPSR3FGL J1650.3-4600PSR J1650-4601?Qyé…¼?TéÐ#Ë4?îe¶þ°Î?«LeÌu?a?©ÀÌÖÖì?ªú…iÚ³í?tÎáXddŒ?}FJ«1b??êá"¦Ð?»-Šƒ¤R‡?ÃÓxŠ¤iœ?ºÝÚJ·©Ç?‰¹"™Ñ@?vPÀõ¡?ꏷßx§?­þ¿®ý§f?Ä%‡J,`P?¬ùdÒ;$k?7N¦–´?
ÿÐí$?ëåe«o`s?£Îßy?Àgbhm«`?£·y†ŸL4FGL J1653.6-0158¿ãÀâ̓ðª@8ñˆÁÛCÀ8Yˆ1'IÀ;ˆ×§b\@ÕºǬ@‹ôÄü?¤gÉ<õSÕ?Ñí×ßO†P@+ÂÑ(| @Åìäo"?™žõµ5¿ÕÀáÜÿIø¿â£ÿYçÓ¿ç÷Í+—]¿î¢Î–Ñh=¿ïþ'MKã-PSRPSR3FGL J1653.6-0158PSR J1653-0158?}ž¿Ûµd?|¦öÓ¬.)?î–)'‰)?®ëàŸIÚ?«'ÅrÀí?¬oºœ!Z.?Œ^NürQ? "®6áÃF?ît5H·G?±ÄOK._Ê?¡¼"àÌrç?¨% ]°b?¨
Üދê?›ÕL™!?ê~Ûb¤,?«ÍáÊ¢?¿Ž›{˜¨?¤ïÏu?aÜyµgöa?UpQâcí?ìó>uÊpç?¡ipF˜?·×("9?¡#¸{©‰ˆ4FGL J1658.6-5323¿ÒGm3×jWÀv/¾3¬ÖÀ8¥èYM‰À;š
oTK²@$$5>{@<§…ëfì?®¢Ç{æ;š?àæ
Î&"@)¨U•:@u—†ÄÖ¿Ó¼¢}méè?¨­1žU™¿ãaΆá01¿ê¥)Ô½\¿ïÿ÷fÔJp?¡j£	#PSRPSR3FGL J1658.4-5323PSR J1658-5324?—ϝËÙEg?" <@û4?ê¬ñ$ˆï—?ÀfSx¸F?ÂRG´aø?½ý¿³¾J?Œbӓ8G?¤HÌi7;?êhÍ,ýö?ÂÊ<ϖêÈ?ĖªÀNÔ£?Á8t_§J?£wâ…>—î?'OJó昄?êûc<2'æ?£gU7i'?¾hôÛÌØ?ŸxQAû›?TùcÊWÝc?Ed–?_?™ÚPR‡X?­¾ÜpP?™£UP¤14FGL J1702.9-4131?äíYý:©?´Ûö5{âÏÀ8t™ŸxÖ«À:=
:{&@vRëŠR)@Æ
c0Q?Ãӑ·øÕ>?á=;•"d@·²ôݍ?þn©›z?£‰£édï?ï ^¿Óêù¿Ý·âYü˘¿ê‰œ*Œñ¿ïÿ§J\D¤?ïïùø?PSRPSRPSR J1702-4128?Ÿi‰¢Ž)?´žçJÔ?éݐÇC?ÆïöӀe?ĜŽÁoa-?Ĉд7¬"?"­Ø«È¡?¦m®€BÀ?ᬿç5M¡?͈ŸW›O'?Û[¢¦Øäµ?Í;'DS?®Ôݕ3i?™lï5¸ï*?ÙâYžz'?·]SÒOA?á!°ùݒæ?¶ÆHÐc«í?_â	\³q/?Mêؽ䇀?ã^Ï&'?»,?Ü\1?ÙÀ
9ÿl?»_Õ2+4FGL J1705.6-1909¿ïÿþ Y|H@)ý‡ÂÁÀ:7/p0ÄÀ<O!Æ#e`@ÌiiP@;ªe™·Í?α%|fWù?ïþx
Ә™@媴ts?ùùu$dÖ?ïòù¢í]?×S"ÜùÀ¡¿âànrb¿ëå#¿¸è¿ê^ëÈRj¿ïÿYM»PSRPSRPSR J1705-1906?³•G‰ÜÏ-?·mê#•?ç͘½µÿ?Ë…îQw?ÆþùD9šn?ŏRÅG_(? ÆòJ×:¾?±ñq×äLó?ìmš^Òö*?Áù£ÆTØ?´/³ãü±V?¸­\^öa?É"¢RÔ]¥?©W± "ZO?àÿà·ÝS?³o‹_i¾C?Ñníhj‡?¬g;G¨EÏ?e'M{Ń?`ã—.{?îô%øϙ?–'‰¥ÉòS?žÉ4v"L?•/;îmA4FGL J1709.7-4429¿é-hGß_À~DÄU/À4h1†:À9qŒ;E‰@&ôî)ô@ÚZæÖc?y5£ •?ÑyQ…XÄè@T8sWæpã@†MZý?¿Q~wÕ$¿Ð›YÂéôü¿ßt†¥ 5€¿ãáû2:寿ë£Q^‹³¿îs'i#°PSRPSR3FGL J1709.7-4429PSR J1709-4429?C¸éÍ	?@Æ1w#SÌ?í,õ¦AG?³†R–¹?¶påð"Ø*?³{öÏRZ?aèbù`†I?_4‹fý?ïoÁ5òe¦?¬'FD;ƒ™?•™Åtª?«ÕÒórWŽ?Š¦Ï"x½§?'óÆ̇ê?é?°ˆ›˜^uÄ?ÇŒ²m‡?®±-Q¤Ì~<Ž¤dÖƹ<»ج½GÚ?ïû€§\vZ?Yöˆâõbá?AýbŽ&'?Yöˆâõbs4FGL J1713.8+0747¿ì[@Lßt@95Ïþ°t§À9­¯j¼6}À<9HW‡¦R@"»ß@î?ý@YŒcP?·"~ޓ"é?á<ñvu¨@ Áòº`@NJƒ&:§?îpOô4ã?¿'ð]À»¿Ä£Ï½íáÅ¿âí ßôq׿îúS] ;¿ïú­z÷íãPSRPSR3FGL J1714.0+0748PSR J1713+0747?z¹É±'TÕ?t#KÈÿÌ?_C?ƒDT;B×?uq´ð	€?w™þ͇îã?‹'0Ÿäì?LÆ?˜y¶?î WŸ‰nw?¡x/-½äø?ž,s¾à&Ã?˜4…ñ2ƒ?"¥¹àÐ!?€dÕkT?í#¤þçfÕ?"ý#Œ"¾5?±àîšL•R??†Hî¯?"þÁ	wÝ?€ÊKÃícF?ëL烀?ª²ÉӖr?À,Ÿß|Ã?§(Ž»·34FGL J1714.4-3830¿îã[TÃ~?¾óÙ@£‰2À7_Ÿ¢ÈÀ9¿¬aó:@ –lŠÂ¼(@"=ÚV"L?¬÷ÃhcÛ?Ç1Ubˆ
{@¡\Á¡ö_?ú|ePç¤?ïééªS%¿ÚŒÉÝ.Cà¿áŸ—£ö¿åô¯iå¿é+܂!'Ý¿ç×ó;Ì^éPSRPSR2FGL J1714.5-3829PSR J1714-3830?ˆ[ÿ"1"?'Uâë'‹?Èò‰šb­?Ä4ªûí-?éb	áê?Ä~!V?pˆéªÁ?yÿë&©á$?ܚrB½C?Ðæÿ=/x??ᑵœŸ.?Ðñb(7?¦ÞӒ'è?" .ûKáü?ÃAbÞª††?ª›ÅèŽ3?éÁº,/Ý?¬S´ =Ž?,Qq%§µ/?HKÃ?ÙVL²Æ˜z?·ÍÄp¡?ãSŠYG?·Ì_aA°Ç4FGL J1718.2-3825¿ï*c‹•Ÿå¿ÜH%EáÀ7	hQ"1ƒÀ:0«¼²@'ã»-h@ÎåD'×?¦(Öbø¶?ÖÃê¥û¨@-Tšþ§±?ñü^]-'š?ïš ri¿×Ÿ2à§õþ¿ä± Hõ½¿ç+
=²é¿îFY¶T»C¿îNõѨԠPSRPSR3FGL J1718.1-3825PSR J1718-3825?fÔú¿èŸ?h÷KQÁ£Ý?íqý	¥'.?ºÐëå"?³¹oÜ׆r?ºu hX?k	új×$Þ?y
÷òú?ëµY»P«Ø?ºÉ¸,	ï?À¾q)ô
?º—ùÈr·*?ªó&–÷?"QÍ\%Û`?é3H#È[?±þ…cR¹?É80>Ý"?°ü,ª/"–>¿û#}¥>»±VSe–Å?îG'2ÒE?šÚøx ²»?«‡œÝº¹q?šÚØ96c4FGL J1720.8-1937?º¸³æ!¶@#‡ÔCédÀ:!4AP,hÀ;´%ï@zîüÍpŒ@ÏBBš¯C?ÊËúêÂV?¾Ê°'Úb¸?÷â™7t
"@¾P7¥Þ¡?ïü6¢(‰a?Ë^7u¦¿êR®ž8¾¿Û`·õ¥3¿æñX½†]Ó¿ïõ=~æìPSRpsrPSR J1721-1936?Îǧ»[C?Àúfê?w¿÷+š´?xþŒ››DS?è–"úÁ{?ÀLÌâ±â?æ¤NDa‹?Ç5M©â?'UnâS×í?‡}Õ£x?Ò$¸®ž)?ÆâµT+9ã?áÕõᇋ5?±´t'
ÀÛ?¥˜G€´?‰²'Tð?Ù±¡4åà?±Fìˆm?怼¾G
Ú?¥­ÙCz?£ë3PÖP?‰×¶ªÜü!?Ё qς?¤ñ´ !¤4FGL J1728.1-1610¿è˜²è¹×@$`;ÄÒ,ˆÀ:S'ŠŸbÀ;ðaXàkæ@³àúVGà@ê%Ðt!?×0y@?å¨Íê>y@/À_A?þ—ÌLÊ3?ØwGà{ˆ?ïôà²\Þþ¿Ä
8èÿ³T¿çÙÁ§Õœ¿ïÿûbâMh?ïÿ<Uñ¤PSRpsrPSR J1727-1609?ŸÄàºmø?hÍ8\í?빩øœ±#?»ÊöQU"?ºA©ÂëÛr?¸©Òӑ‰'?ÂÊܝÖE?ÆV3h
k?å‰Ùn›Ðô?Ð1R‰y:4?Ç
½¨åî?ÃËäãñb?Ä®Káw?£íÅð…k?á<åC§Í|?±¹¸Ãbú)?Ó/+S&ôK?¬š
®`?£²ˆMkœv?'~hmúµN?æRàñ|4÷?Á$L"Ý"?ÐãíZ"ƒ?À'Ðlãu;4FGL J1730.5-3352¿äßøVF?°ÎÃG
IÀ7⺎ç¡À9Ú׊•ð˜@j±UXL@½ÀÛ'£?¾»+ÿQC?Ò܌=:ž@<ewS@H)Âq)8?îúæ ³iN¿ã5'»0¿åÞv½÷qç¿éª<P¿ê‡¡8¿ïõ|RÆPSRPSR2FGL J1730.5-3350PSR J1730-3350?'$¤.¯…†?¤rÞjËå?Ñ¿ÊI'*Y?Èfº>`Ŋ?æ–õ¹Án§?Èá ²$sD?‹<‹ò总?Ž<1¬¿?Åú'Úâ+´?» ‰×ZP*?êi{Û?»*¢3@e?©÷Q˟ˆ¤?"Æôà'??É6Ïá«Àœ?°M‡7¯Î?èÖêÛO?±h—Ñx?Y¤_ã¹ÒÞ?HÄ֒<S?Éþœ´k¶?¨³ƒ
Nï?és†¢íÈ)?¨·	t)Á4FGL J1730.8-2303¿ïî—óÚ¶M@ÇŸ¾vÉÀ9£@4£vÀ;AÜ@W@†ž^ÐDü@(3àØŒ?ÉÓËñÛz?áRíãÉª@;ç)oe@yÙú1ßÌ?ïItR¸3¹?ïÚyޓHÈ¿ä3ÞSÝοë
`z"¿ïþBžHU¿ïøT¥sÂoPSRPSRPSR J1730-2304?Éw2<\M?½«¢­	?äTˬRæ ?ǔÜnù?Å5ŸXr?ÀD	ùýt?°È㏔?¹0þíõ?âL
ûÀ½?Ð
à:?×5悅¢?̱°Hºy­?ÂønÌv?¡èÄý ?ÓNL3û$[?².ë¯Í=?á§ëÊ~:µ?²€oí˜?ŒHæKD¥?wT¦±.]?æ´¹4mŠ?¶ùkf¥D®?Ñ´Fe…?¶J¢;ð³4FGL J1731.7-1850?éüýùs'@ ÂÀð À:;ô¢ÕÀ;ÐÔÚ¸GÛ@öÀ l8@­±™jŸ±?ÎðʐÀW?æ¿Û¢¨‹û@­¢™ó\@(ÿ#·T?ïõ桊(ã¿ââ÷Fÿä6"¡¸!¿íÅWïnb¿î¬ ‡t~¿ïPk®ŒpPSRpsrPSR J1731-1847?ž
¼}?›éÑÙûÇ5?ºÄœæ·™?µ\þ|6?ë·už<$?·nýTOf?Ä°	µœt½?¬¼JçªT?ן°Áÿ?ȘàŽLr?ގ[toƟ?ÉGH–4?Ò{'<~Õê?­fæ*d8Ž?ÒGìcðJ?¯ˆÐzz—?Ûr&×9Ë?°TšY7Ý?Äk|*@E€?¡"O'æ|?Úo½ÉqÐ?²oû"Þ¯?ÛZ"!Ìkp?±[Ìx.—4FGL J1732.5-3131¿Ð5°œÑ˜ ?ðã†Lµ»À6ioê›ëÀ:oE	@OÁ^Z@|¢}méè?˜‰:%ë¢?ã/џ‹A@A㦽nŠø?ûȚ$W"?ïáKª"}Ù?Ðxoþ?¶y¿ÑZ³ɹȿãÔÐ=0ã¿î.Ö­ _¿îË¥»PSRPSR3FGL J1732.5-3130PSR J1732-3131?«¥ä&ç?0Pp³?ïßþBðú±?v‰sìóà?o"wt¶?v:´Â²—?WúˆV@ê˜?löªÑ¾Ÿï?ï杀ÔÁ?¨ kÔûœÑ?ãƒÊY?¨'{Ä7»?|¦c³ª?aäK¤ã¦¥?ín¹«'‹Û?"±ÒX+*ï?²¿Ìk'†Ž?'ÑîÑÀŠË=Þi9ÄsŽ=òwe}§1¬?ï÷¡
×u"?R$ãªøñR?P½ê3qf?R$ãœq4FGL J1732.7-5050?è6jÀñªÛÀ"énX£/EÀ9×ò<ÉÀ<2³àl¼Â@·(@7`9%»{?»UJ	c?Ôßs㧄¿@¢;ÿŠ@ôöw5F?ïø€_5ð}?—Ä֚g¿Þ|RáÏ=j¿ã®ŠÂfA}¿ï7iÃèø|¿œ}ãä*ÁPSRPSR3FGL J1732.5-5048PSR J1732-5049?ÒtLê‹äY?Â÷Ó§&?á¯éé'Ù?ÅhôJæÆ?ÄW¾†KÃî?·üïïf3?ÒãBžã e?ʆcSt?ÑíÒÖ²â?ɼËIÞ[š?ÜώF,¹?ÍMË)28?ÔéPñ¾úà?µ
Àù»™[?àQ*½Ì?¶ølÅD9º?Å°tc?¦*…úa͂?áY&oÀÍð?°+vphQØ?Ô>"КÃ?±¤|®Ii?Â]û['¼?¥,³˜p3®4FGL J1739.4-3015?ïü£ë@?Üã!M»À8¤i×4/À:†ð¬¥åØ@øèë¡@âEõ­–§?Ä_|sp?ä÷—{²(@¿ï|$=Í@nCG'†Ø¿ïЅžºë¤?ïüúz…¿Ù#faˆÜ¿ê@þB:¸
¿í¸^_Ö¿ïÿì´É ÈPSRPSRPSR J1739-3023?¤S;½}-?©<©'€Þé?éÌF¶é‰?Ä5ÅÌo?ú%þ4ú"?Á5@ËqÖ?¹E½ØҜ?›uì QÙÇ?æu÷€\æ
?ɱ¤¶_?Ò&FÑWmQ?È(Ã@7Î?­G¹N«›?–ížFk#Ž?âvŸxù?µÜµµ?×ißIæœ?´\Å0ў?y€ŒIðÒ?d1;oˆÂ^?äé§8‹2?µ;ŽM?ÕÈ?Œ¸ÇÚ?´ÌÀ
¹"é4FGL J1740.5+1005¿íPœœû›@4EèÄzôÀ:ý©äjxÀ;ص–Ob>@Ìò"l`Ñ@"à??Æj©V¥ÿ?ÉF…àÕt?ú˜äÓSϋ?ücñ9Æ+?ïýÞ½ç¿åԅ=l3¿ìÊAR¿â&H3uxR¿ïútpe¿ïŽhþÇÜPSRPSRPSR J1740+1000?v÷?—÷Ò8>L'?…;mf?ƒüûbԑ?'!톯Ô?"o³¶Bè?æ*…߁á?Ê$o7øÈ?Ä>x"?Åô|€?Ãæƒè?ºû0Ýùã?æà°.ëB?®ª(¥ö=I?±ÞZ\*?šsQñ?ˎ–=æ?ªBó;Ú?Ý*&"ðhô?¬S—2?͒D³4¹?¯?ÆeEÌÀ?Ô·u:ƒ?­Ì×°ñ›°4FGL J1741.4+1354?ï.@3"ý@5«ä›«—À:5òý¸ýãÀ<O)õœÏ¯@å7¿)Ì?ÿ±a‡"à?Á¥[Ä¡Û?Ü	`{ë´@ .s±?þ©l$ìH"¿Í®Ñd65q¿à³xgðª¿Ò3Ðý^*¿åIåý{¿ìË`P¢¯Ã¿ïÿê0ŠâGPSRPSR3FGL J1741.5+1351PSR J1741+1351?Àw]®"Á?´-H~;Z?ê+dÎd–«?¹Äš´Š©õ?«mI¢þ
Q?£^ùiÓg?äÂø¸?¾~NúŸ?çiÖ
ۆ–?Ãè'+F?½gËk2[-?³©'pÝ8ò?»èâ6š½?£ßڅ*ÞÁ?ç—B¼–yŒ?°èBk~!?îƒò Ls?¥^Yˆ|Î?ÕGÄ7&9•?«	gÁìh?Ùñí9?²ë¡A2Í?љJ8ÒÙ3?©tÇKÑÐY4FGL J1741.9-2054?ﬤßPš@Ÿ@=ݱ!À6äN¼üÀ:Á±RóÂÛ@%'cœ1¤@)õ>ÛÝâ?š¢x²¼?è
U¾xv3@C¿ohی?þa3™Š€!?íúՉ3ðÈ¿Ì8èê9Å¿âOÅÀi<¿íu!À5¿ïÿ¹žœ¸³¿ïÝ6LJ[PSRPSR3FGL J1741.9-2054PSR J1741-2054?Mr–¨·?RNßôµÐ*?ïR‡É€™?"ìÞ·TG$?"Ö‹rK7œ?"]î iT5?cªÓµ'¡?~ç°¶^ßÊ?îåq9óŠv?µ"•¿¾3? n?%nGû?µt®D"ñ±?•-Ç}hêÈ?Œ¨‡6ӌÐ?ëŽR ¶ï	?¥f…YOŒÑ?¾AýîM?£RƾæÀ=çͺ45Ó°>
?ò½e†?ï÷Ÿbмæ?QÆ:túõ?PÁ:.êÀ·?QÆ:\eõï4FGL J1742.3-3318¿ã¼hÈZ;$¿ûÚà‹ÆrÀ8ÜkÝËùÀ;/:Wꢡ@ŝ7³Ët@tEêPk?Â|˜1º?âú'
‹þ@–¿Ê…Ë?þ=šOw¥¿ê}©Æ˜?
Gç¿×!³ƒûw°¿æhwM>w4¿ímpEã9 ¿ë&€IRPSRPSR2FGL J1742.5-3323PSR J1742-3321?ew$Œ•?^PJƒ"è?î2vðš?¦OaÀ
õ?«~ÆÝX5f?¥ÔÊE bÂ?†É¾1µ?'ª›0ð?æÓyúÍJü?ȋŽNCK?Ñ¢Ãüt˜{?Çú7æ}Õ?¡¤ouû'<?…ÈÁÀCš?æLX½W^A?µ¬d5UýÕ?Ñ2À–'Ñ6?´E%µ|$?rö 
·?[ˆ
Q?êójÅÈ?§ä	P)8‰?ÄóÏ1ì@x?§™Ù?Zý¥4FGL J1744.0-7618¿ïpñ"_üÀ6t¾ÆyÌuÀ8¦-vZÐ0À<óý">6@˜rÆñìl?ü̲{ï?¨4_>e&²?ã8MžïCð@3Ö}sÉ?ü'@³½?í¸Á>#Q?ÔY3wü'¿ÕfŸÜ©¹¢¿åü­_I<¿ï¡±Ë¿†"¿ïüûÔ!TäPSRPSR3FGL J1744.1-7619PSR J1744-7619?w«>¸'?ƒ'ù>ªÎ?ïnžŽ,Ö?#€µ§Þ]?ˆ'ÓÕs
ê?"åR®Ìö'?ŽÌkƒúŒÝ?•m`=þã¸?î`(®"Æ?ª[EÉG6?¢L¢"{?¥€AšÀ¡ž? dØçè™?wÈ*7Øá$?í-¬1ÿb?—(•ù?³Ú†SÓ?– =>îßaAJ‹i>ìÿ\b<ï?ï§vðJ9?w¤é¨éJ?†5*k§?wànÉ`‹4FGL J1744.4-1135¿ãR,þ:Øï@"]·k;¸=À8r¥®À;T¨ŸÆÚE@¾õɛ?@õ\Rç-¡?§G3¾/?䦏ãW@3áœàu÷@蕫"ƒ?ïþ™côÏ¿·üæÅò=¿à-1üÒN¿êꛟƒ=¿ï×ßÖjÛ¿ï÷ß4®]vPSRPSR3FGL J1744.5-1133PSR J1744-1134?p¸eüŒ«?w©Ê&:–?íYäŅe?·R«gyWØ?´%St;?¶'o|Ñ?|ŒæÀ'?'§ë‡ùM@?íÑ®dSù–?¾§ñ<V®?¯bèüΕ?¼Þ"î<]?ŒÉ-bô?ᯡ¶C?뱓@‰œù?£I,­6Ü?¾Ú@[&¹·?¢H7™ð»>Î}WE.>Ìf™#¥‰'?¼eÐC?x¹"´
?‹ÒéÆ~Ë?x~ѤjÕ4FGL J1745.5+1017¿îs^V¢y@3>­-ËfÀ9šVÿÁßÀ< W¯ê=÷@VWwá
!?ÿFôæÇIÖ?¹=uai|?àE=V¢¤@ 'ÛçòÃ?ùð:æ?â'!,öX¿ÜX°»t4ۿӍÈhûí¿âä
k"ÌÑ¿ïÉûa4Î>¿ïÿH˒:PSRPSR3FGL J1745.5+1017PSR J1745+1017?€Þ-ՌºG?{>(îjY?ïõXó?…:S&¬?wHÕ¨å
?uDœ§?"Ì'ÉqŸþ?¼v
Ç?î'ú7p4?¤P|T¦?¡7Ûì"Ê?ž*N¡–aÆ?›áï¬mê?‰­ËÕNï?ìf´Ÿb?œ?C,ð«b?µÑ÷	¤M?—;jlL)¦?"Vµï
?ó?kíðˆãs?ë&$Ty¾?¦êF/­˜g?Â"›½E?¦wàp¿€4FGL J1746.8-3239?×öb›3UKÀY1¢9{LÀ7Ãu"*ÐÀ:ïoɼw@M,…šT@o<¥¢¼?°süPH?àÿ»lR8²@0¾ß¤@?÷ ÌäIÁ?ïë)yv
£?è)8Þm߿ݸõ_='S¿æ°ô>«·S¿îw.4Ʊ*¿ëˆª"¼àÆPSRPSR3FGL J1746.8-3240PSR J1746-3239?b)n¢¼^?s"àÚbS?î»cÌÖ9ô?¶þ
¸Q¨?£)À›²4ë?´ûëÞqŸ?nçJ[KÎ?€˜o]ʒw?í
!¢ôó^?´‹,…ä®â?¶Ÿ¸•~?´3™Íªo?ƒ"ç 	³Ž?nZ邉Œ{?ìïZ›Á¦K?˜ï R—?¶Ž-ñ—6?—VL?.Ê>ÆÁ
¡–Âæ>Á6£!?ﱉWî½?umøÛû̦?ƒ¹1™Z7m?umBm'BK4FGL J1747.2-2957?Ù
ŒbÄú¿ë
ßòC~ÛÀ6'Ôº××ÃÀ9½åëoO@ÚÙÇ1@Åûø3ƒ?¤RRá#q?Ø^TùM@0yJ€à@eݶ•?çS¼_í%ˆ¿Ô¼"E$Lf¿äjšêÒq¿è'kí"¿îCƒbu–¿ìùÍ¡^	 PSRPSR3FGL J1747.2-2958PSR J1747-2958?n±fäɪ?ord0ÛàW?æ·º>nŒø?ÐðœK鳏?ÒS(µZ¸~?Ðçk8nò$?r¸¬ƒ¾´{?{¢Áxœ=?누ÈÛ­s?½¶ñç>6?ÁH'xsT?½[g–·=?˜ð}üæ¥?Á"ÀK\?æ1~¾Tk
?µ"'p"éß?Ò{w[€?´,çÞ¹]W>á¸Ù]r*>ß
OÕϲ?ìÁÝ}çg?¤²=÷?¹ð†IûÞ?¤±ÈPÀÍ4FGL J1747.7-4037¿¶Û,™¸Ž¬À¥P"WBÝÀ9"A!"µÀ;ϜÈù¶@,ØCxz»@ŠwTË?´–Õ™úèi?ܘÞ]ÃՂ@"'6¬dwy?ÿü¨G1lß?ïÉ%x_.¿Ûz1¿•¬¥¿ãFÓ#(#¿æ£»-h¿íœ=þ"Ci¿ïüe¬,CUPSRPSR3FGL J1747.6-4037PSR J1747-4036?fß]nýÕ?`̞™~õV?îÝ?ï"í³?œ!´¶©? ¾/ÁG•?šÅM>uŠ—?†ç7Úü?Ž€|jٔÔ?éh+Ÿ§?ÂÔ¥D'Nc?Èþ¬Þˆƒ·?{'°¥?¤_--á†?'uN00?ê×iü°?¤Ðëƒ,£?¿9€‰3ŽJ? a«7ÚÁ?lRJl×~?T$ðá l?í>uòŸæ?¤06à~?µ,áûïš?W$È]K4FGL J1757.9-2419?㏚µ"Œ¿˜K?™s-À8xh¶¢¾ÜÀ9ø#CÑæè@ 4ÇÞ%²@«¨?ùA7Ì¿a?ɳ‡i!,@S™ V¸@d¡¼'ãõ¿¶ÍgÑöW?í»
bY'l¿çæ a3÷¿ê^˜q{m_¿é*qš!¿Ð1Ácb%PSRPSRPSR J1757-2421?³p2º|–'?µ"®XV¡?ÂÖuX+ƒ?Ä	xt£6?èÜ\R°bZ?Ç¿ßÌ¢—À?¼™ñ@·?Âù…"ÖÄ? æ,⶗?°hš·_Û?ë^_	Ÿ£?ÂùÀ¦°æ»?¹¦íÇq? \9s@?½Ô©€™–,?¤/£<övm?é	,ì?©Ò։ážl?®N^P˜u?±öœ>)?AGåہÂ?{éSD¤4?î9 ¤?±#Á›¶†%4FGL J1801.2-2450?áŒõ±Èdˆ¿íÔPXÝèÀ82ÿݛQ*À:šÂn¤ù@=öÔ{@B­Yiþ¡?µÚÎ~cïO?ÎÄ»Ü9§A@>¢Òþ??õåC¼s?íÈDÝ¢x¿ßÆ:ÂÇ;¿áõDD¿ä¿T_™¿é…¡—û¿ïÿ&PÌ¡.PSRPSRPSR J1801-2451?š8{@º?'`U\DB?è3%§å6ƒ?Æ7_rÌ_¼?ËìWqà?ÅsO56?ƒpè|p?ˆ–½Œ£,?âò{ÖH?ÉlÎ( ²å?ـGÆJô?É*Ùј?´ðYœàIˆ?›:Ïk–«?ÖÇìäÀ0Þ?·')ôýÎ?áýþZÞ`?¶‹ÐÂ"²¬?fRì›Â?O+@…!ža?âoØæê<?±ök$ÖH?Úó¨XôÓc?±æòìGí²4FGL J1801.6-1418¿ÖðW'Ñw¤@Äk¬÷DpÀ9ß%"åÀ;ÕWµÉ{@Ə§þ6Q@3ƒB??±?Лl¢À‰È?ä›@ãŸø@kf¶~¢@_s"\³?íYiþ¡[/¿¾ò\=îx¿ê5ŽøU瓿î],áŠt
¿»ÂÚô¿ïÿðÇô PSRpsrPSR J1801-1417?Öa³u:_;?Åᜋâ?Í·jõ'—?Äýœó£˜¸?ÛpÕJ×z?Ç븐M*ç?ÆÉFkEX?ÀÊ0Ë­ª2?ÅW_ÿ"…Ã?ÄÛü|LÊ?ä÷áî€M9?ÆP©Aþ'?ÐUp¦Ž….?«[	ho9?Ä|Ž\R…?©Ú]£æ?âÑ(‰!¨È?±§µô)ü;?¶("°À¼?¢V)úÍ?ºÝèAu?³¯6%¥!?éßI¨jõY?´ì€€æ4FGL J1802.8-4719?ïÿîÀ^øÀ(qûÅޜÀ:šÉÓIÀ<2w¬ßÇ{@ÃßóE1@@˜ü»§á?Оˆ@Ö´Ø?â9Ž—@§ôÛߏG@؟ÎçÚ?ïy ÕÍýN?ϳù—02οâ¡sîeô¿éÅ# ™5¿íŽÁ.32¿ïþ"ÐÜýPSRpsrPSR J1802-47?çu"׬¿¯?Ĉ}.<?õ£ï:--?¿º ƒFv?¼ë¡d%¨5?º{Ð}ø?Øe·ÐDãc?˝ý´ë
?Òöêžé-ç?Ëà6»`+?Ô£]Ñî¶?ÈíÔsìÄ]?â·÷è®È?´>£…\\?ǯJ]<2?«sܲš±:?ÍpÙK!P?ªO2ד`?Î[¹á;}?©.IÜ.ñ?ὑF2Ç	?¹7׌	ˆ?Ê®ùfÕ?µ®•Ä"͆4FGL J1803.1-2148¿Òzª©iùÌ?Éx.û@'¸À7"èG|–TÀ:´v"±Ó@çûZ(ë\@µô^N?¦X"Ãs³?ÑÑ	\õúC@%DæŠ
5@½í;WD
?ì­nB}Óë?îè* dú¿à;­àÎaw¿ãˆP›ùÆ*¿ë˜K$Á€¿ëõe<š»PSRPSR3FGL J1803.1-2147PSR J1803-2149?]ŽBÕcN?XÚ&;•Š ?í¨YÕ!Ãö?´Ÿb)¯?²HëæŠÅ?´d®iú×â?p¨1&nÐ-?wÇôþ
ς?èŸvèô4?ǔGù÷ð?Ï@›(¸¯?Ç£ýDå[?Áxà/ò?&LE­>Ü?èŸg¾öz?´˜Á™†?͍SDþ'×?³Ãpv<Yë?.Ép4Ø,? {ÑQ Ñ'?êza
[ï"?¬VWñ˜2±?ÆÉzƒç?¬PÐnÄG4FGL J1803.2+1402¿ì%!†@)@0êkƒÙ^À:˜û܄еÀ<[›]@@Ìxé÷@Ò¶»éOº?Çâ·ðœ¶?ۘjû .@Eâb`Gh?ö±Ûø8áH¿àfç?¿³Š?tÈT0󁱿á¼v¾MX#¿äHb°Ï@¿ï²äXڌ©?ã÷äþqàmPSRpsrPSR J1803+1358?ÈÑóÝ5Ù?½M£«Ó?Ú?܍kûb?ÈU t]³æ?ÙW)ñ%i±?ǐNG'¡…?ÔÁ¯"á?ËØExm?ßÎr‹Tÿæ?ÐIÆPÊ
—?Æß¼£"þ?»–(?%g?×mY¯•6?²|"ðuÑe?×xù¯4?´Ç	…ÅrÍ?ъ¡×qI•?®cJp›á?ÏP/Œ=ö?ªÖ¢)?ڄ³Š†vŠ?´'@ý±e	?Õî¤]³jz?°¼6·°4FGL J1805.6+0615¿ÖÂÓº&×Û@*΅3±À9öÝpˆÿÀ<1#|
Ü@Þ~Û¨1ã@"à¤ðæ?Áw'iP{˜?à"<›<@#VSÉ«°@ßT¼oÝ^?ïâp"&ñ[?ÀÏÅ0¡¿Óª;½ÆI¦¿à눯fŠy¿ïÿ©-‹S†¿í£?O¦†PSRPSR3FGL J1805.9+0614PSR J1805+0615?¢cÖkí&?¢ÿ¯Úqª?î6^­«'k?ªy¾OMz.?"l}rÀðV?•Ü丫?¦EÆ!<?¨ãaµÖŠÐ?ë]ƒd–êæ?¼kGë|öò?¹ñÊÆ ³?¶Q'Î¸ß ?ª8¦…5s?•BÈFÛÑ?ê؝Æ,&?¥b¡/¤‡~?¼·+¾Œ&?ŸSǔ?¸R…wj?—ܲ7ÝE?æé5ÞäUV?®;vUɏÞ?ÈPšÛ+îô?§û-0ñ4FGL J1807.1+2822¿Ëú†'vç@5‡,ƒì‰+À:£àyQûÀ<2È b@4÷â¥&@á'©?͵ûåi%Þ?Ê®¢jM¦§?ú†¦\ö{?ó™–dïï?âqíþ ¯c?íØ涂޿é8h\	ì¿ë(0Àè#¿Ç°I‰`çK¿ïÿb¶®}VPSRpsrPSR J1806+2819?î%¡Ctò ?¦~¶æ¯˜ÿ?"i@!öX-?'§B@ك?¨‹›À3Gë?¤Ï·Dœ®«?êÏéÞ˜ô?¾b¦=¾¤?ª,Å\î¯ü?²OÅq-yn?¼jN`›à[?´‰aP3¶?êàCãÕÕ?¤½¤gSK?¡OfÈz]·?¹P'W§?À+ù>R=? ß‹äH?æ‡üÆ>ÈÐ?²sCìÇØ?¸¤zšü?®k}?Q¤?Éӊ"ǏA?©»³U^–®4FGL J1809.8-2332?ܖeâÝÛ=¿ÿóÔ
2îjÀ5˜µnvÀ9²æ[L@ÔQÞÄñâ@ܕà•×?½ÅüV±?ÕÕØ#ÂýÁ@F-¯ ê[S@''[²ƒJ?ç´4ºò¯µ¿Ïñ¤ƒ³ÿ¿àÞ°z¿äé^¾Q^í¿ì¶óé	¿íI³bmˆoPSRPSR3FGL J1809.8-2332PSR J1809-2332?*vF—0}?#u^
S?ïfèW6?¤EgãP?"ÖgÝø8?–°Çáz?\%‡à>Û?pׁ!á‰õ?ïU–~÷?£C&9x?"œ#?¢ðGÍA÷?yA?Ýb{?fëxaV²?ìÉH®*½? @Å`½?¸Æ{Óí?Ÿ—Ehá0Ä=ÎaIu"%=íCH!¯•?ïÏ@žÇ_?ÐÇi¼¸C?x_°˜"?ÐÇg³|4FGL J1810.5+1744?éCr2Í\À@0ÏîÑížÀ8(Àéi¼À;›I²Ñy@fúÅX8@Øu'ST;?§L&Ÿ& {?҆µ¼:…@%p÷…@ÖoºÜµ?ì÷ì5Gài¿Üd…üðJ¿ãÌ©C6Œ¿èä"ŸR¹¿ìô#ˆ›D•¿ïó!3FPSRPSR3FGL J1810.5+1743PSR J1810+1744?';W7:c ?‰}»>ûI?ìn|±ý3ù?·³ ¥[k?¸=D¢GÇS?¶ÖØ«B?˜;'L^ }?¬"É5v'C?í-d%ï?¼_¨ƒÚJ?°†$¿Hd?µOû?Ês}?º¦Ôðãï?¥,g	,Î_?èsðÎ8b?®·Àd?ÂjÅÄU"?¥'E¹1J,?Jçh@ž?wڛ…O¶?ë±ù›9ƒ?¡Áo<8K?¾ÎOù+Ô? òï[.]4FGL J1811.3-2403?åÚ¯T}ÀWg?ª9ûÀ8µml%QÀ:'
©§-×@ ?z¿8å@{Ú¡¡¥Ø?Âü$©,µ?DZéDŽc|@±B³÷+?ínÀ	šÞh¿îÌÂn¤ù?êðL-Õü ¿àÞ	|¿æ°¸.°´¿è‹X=®·8¿êGM1:ÇPSRPSRPSR J1811-2405?¼‹0mñ?ºŠ2ò«%?ÌrGó
†å?Æ%…¦´$?åRïºÉ?ÈfØzۜ?£8"Üô¿<?©Öqeçûs?ÐMÞx£?ʸï=^%?楎Ì&÷»?Éå8J{–Ê?¹ËÔ\êUØ?šBÂ	Ç&?Á¦ëˆ-R?§X¥_/?è\ʒWQp?«¥ÀVœw@?†ŸRj·¯X?q}X­M?ÌHƒ·g?¯ÚÂíLð?è"Rdsi?¯èãí=4FGL J1811.5-1925?È$Pj¿×$2#é".À96"4ÕËÀ:z&­é²·@!Ë仯@"Á¨¬\?âA{_ò®ß?áL!¬"2Z@«ã	O4@Aý#,?ç…"~°	¿ïB-¡ú?î•TûÚ×R?ä˜Wz:¿ä…"ÿ‰b•¿êî~F¬ãPSRpsr3FGL J1811.3-1927cPSR J1811-1925?šËô%€FQ?™wᯬ+?r?EßÙ(?yˆ9¶àh?ï!Ô¦>?œq,ڜë?dzá5ÖúH?ËP'#j'??ðˆ®I?¦ÅQ}½?é'.DÏ!?ÊßÄïugI?ÅÅ2i¡k?¤fªNÅÞ?¾"'ã,x?£'´k)tg?æ¼NiWr?©Ð‹C˜Zý?´·²²êxñ?´·@€(?z1ý³Rz¹?†?q
Œz?í4¥®<ì?µ°"wÂh4FGL J1813.4-1246¿¡Ãã9Îú@Š.ÝcÀ6×1ªœ÷À:O"}Š@öÃì(ˆ@?_[°)ÿ?'D$z¼<d?Ôª±ïÑ´"@<ÜÇÀôQv?úû]ƒé¯?Øhà¿Ô¿Úâ'[â©Ù¿ä²)³W°Á¿èѵ¿¿óö¿î2ò yI¿ïþ Eð¥PSRPSR3FGL J1813.4-1246PSR J1813-1246?PwúP‡H÷?UÀ"`KÓ¼?êåÍ^5p?ÊMÆêÏÆú?ÄIÕæ¨?ÊAxÓÂ1?^QmGe?o¯wp"†|?î8t#$Üv?´c n,H?«†2cy -?´Aì¶í)?˜&ã¿Ý–?pî ;¸Û?çŒâ3öS»?³w·Ì€'~?ÎǚÏ.µ]?²ŸYHþS‹>W†Ñ5>b/#½À "?ï€115Ø?…Š4¢.·-?ø0Ӂ°?…Š3¤)ò4FGL J1814.4+3132¿Ú8œNT̶@5²køvŸÀ:LsGyBÀ<&_ċµ«@iº-ã¾@÷òeÊ?ĬÂkIû?àW.ºþn0@±¬Þü+@†Ð.C¿ìw6b'œO?Ԁ÷Áíö"¿á³p:$¾ü¿ãˆáá¿îÞ>s³¿ïòýƒMýºPSRpsrPSR J1814+31?wã(ó(Âø?vq¼×c2?ïO0ª¢?'&[çǾª?! Œ»?0۝}p?® í	Ÿ/~?¶¡Ñç÷¦?ëåÆa‡¾`?À燫4ø ?±Vnòu>?°.'»"?·	>Oþ‡?û© ìn?è>lˆ³?ª/4d#of?Ã|É>Ñ4œ?¢§?Ó´ÜP?¤$5k­°Z?ˆý÷ìé?èÕ¸žGõ?³ƒÁ"í?Ç ž›t?²sG1݈v4FGL J1816.5+4510¿êò©g0Õ@8¼`ˆÖÔÀ9O¢ÓÔþÊÀ<Hm'ÓÒ{@e}x£U?ý¤y&\‹?°!ñâî¢?ØOŽÞ§«@$­1ã§Û?û˜'©í?åÞo÷ß ¿ÑUU|´0Ÿ¿ÖXZ_=¿åW¤A=b¿ëße‹u¨¿éRlžä²PSRPSR3FGL J1816.5+4512PSR J1816+4510?"9¤_Å?Œ"¾*F?ìÍÁDŽ›?³Ã˜º–C?´ÈðÞ{?±RB˜í"ê?†~'"¨è?èÃÖ} '?î§4K°¶Å?¦Šäë¯=¤?ŸÚmÀ×Òú?¢›C¹`Ö!?›QÆÑ­¢?ˆ$.â<á?ìþ|2g?¡®129F
?¸Ø·¬¸W­?øVƒ3Ã?ˆM«C>*Ð?uÙÏç.?ìV¹7Ðo?¢V0—p7?º@€ÙÁó? úèwge4FGL J1817.1-1742?æòI0ÿ
¿æ¢1ƒ/ÊÉÀ8Xw…À:žé|/üG@侊ê™@^¯ûÛ®?¹¢e^î;Ì?ÚL®ÁI@Åðáy?ùžv*úÕ?ïzÙâ)U¿Þ×q@ŠØ¿ÞƾÀł¿æe}'%¿é™ ºö
´¿ïÿý`éNäPSRPSR3FGL J1817.2-1739PSR J1817-1742?•kuíäS1?ªów±¥|?êBe†'*?ÁHG'`.?Äý‡¬*Øñ?À,rh%v?ˆdì9Œ{;?øä¯Ír…?á*V
Ðeð?ɋ`jÒg?Üè,ˆ'ÐF?ÉN2ó"½d?¬I%÷Õr?'ñz…oxô?ÝIï´¤Ž'?·?"M‡É‡?ß,ðœvÁ?¶kQk·är?mœõæ7®?RÝ$j¢‹?àٟjÅ;Ê?°«Zb²8/?Þ‡>©qü?°œþ;Vp4FGL J1823.5-3020¿î43ÝÀŒˆ¤~ÏêÀ8üŽ~³dFÀ;ðåÍNÒÌ@H"Î;G@4²ú"¯u?­‡€sw?ÒãÚzµRÞ@ C­Ò^Ý?îŸ)º_¯?ؽa4"¿ÙØWdÀÉß¿à8lXï¿ßÓ~—µ"Ë¿íÔ§¢òu¿â#ÎÜq…~PSRPSR3FGL J1823.7-3019PSR J1823-3021A?€¶lì³?¦ê8;ã…?íÒožYÃ?²¼:P ?®«jú/c?«É¿Ð°ÿ?ˆ‹(¾ëoï?"NŽ¿KjQ?èãî3ºn?ÇT-¢Ùšµ?Ê甥)GH?Ə$"÷ë?ª/O‡å¤ú?—õŠfP]ò?ê¥lÛª?§gÀXÃ?ÁSՈS(?¢¾Ó"[B?lŠú¨Òé?W"M`³i?ìëá–hÃm?¢"?ì0?·¼›wsMR?¡èõšR'4FGL J1824.1+1013?ÊÖ\'k@%NÉ:qÀ9»Œƒ"_À<tЌu@Hkԏ@c—>?½ø^öÛi?Ö"›Á,Î@ýKÁŸr!?úT"úP=°¿äª|`"Õm¿Ú_3Â$RE¿Ü8×¢hË¿áîg`¿î*= ÿ:¿ïþÃNžÊPSRPSR3FGL J1824.0+1017PSR J1824+1014?¬<Ì£:få?¢I¾þ7f?饧ZÜÏ?½ïm7
¹ê?ÂZ/k¾*?¹'NûCš?±j,£U~r?µ~üúèº?èØ#`ywæ?Èrõ¼÷a±?Ãê\,oa0?ÃoÕ0e?°ÐŁ6-@?˜'`èmôï?èÏÔÙfÈÑ?«ÅC°3H?ÄXIÙÉÆ?¤ì³‰ÜëÖ?Â>!3››?ž#€Ô½¼?Þ¢ŒkÔí?³fE*1H?Ø>bú^bD?°ÏTãPªÔ4FGL J1824.6-2452?§sÏÙbÀfÕ °åÀ81Må"À;6ÕÓËò@ùmqÈoE@=">5ŵ?¬Í`né?Ößf'¥"@$\_|gZ@Ø¢' *?ìå€UÐÂ?Ëoä¿\̵¿ãN'¯rHó¿å*lO´s:¿î™l¸þæ¿×·b|×ÂPSRPSR3FGL J1824.6-2451PSR J1824-2452A?fß»¢:ýY?^+¥X±€%?ì{ڂÎ?²$ý"æ8?»j.}÷s?±ÙÒAÀÝ?…í+ýóea?‹áÙ§w4?éß}ýH•~?¿"ÍÏ«¼?Ç#5Jþs®?¾®™%Gîà?'™Nš+T?~Àgé¶?ëÓgrëï?¡¼Ï|‰Ý?½ÝÙý?ŸYû÷æaÉ?qVXâƒ?Z4-^ðΗ?éèh<•ôN?¤P?ô·?ÇÑtZá±?£Ë>HŒ•Ô4FGL J1826.1-1256?î¢`_'5¿ØžžôÀ5°¦#뗓À9:FÖ~&w@Šp8ø,@Ú j™Ò?•4Ú¼P?ەn¼¡0'@@ÉrGE8ï@ùF'¤?ïþ"ÀC§u¿Êzأŗy¿àüDôü–¿¿æ"x'Èœ¼¿íøMïwÀ¿ïÿÿ&¦³PSRPSR3FGL J1826.1-1256PSR J1826-1256?ÁnÒá‹8H?Ò°H®FH?ê›àø¡?Óms!¿)?¨Zöyc"É?¾®PB>W?X`!…²â¡?qÎÅ·d{?îÕäQ
S»?«YŒíß(?¡Þ¹âý-8?ª¥m»²±?þBP¼?zãHµ@">?ëòV?ª]Z‡«?Âêô•=Ç?©RUldù>åÊÑ>…jß5¦?ïpªN¦kï?|àèVÇN?'ê¶)t?|àÚD¼Š4FGL J1827.4-1445¿Ç
óŒîÕ$¿ø<äŒ×êÀ8cã\[J©À;+ÞUõÖ@Y\·Ý@m²¥Ú¼?¿K¸ÿÕ&§?ïÿójÆGx@#ØÛÎÈO@udǪϿâMš¢®R?ï9žÝ%`¿Ê²wa
†í¿ãÝek"£'¿ïùãñ¬€&¿ïþ䬽bÌPSRPSR3FGL J1827.3-1446PSR J1827-1446?f¬¬":Î?w‡Ñ…qÚ?ïÇë?™Ò²ÎA?†#|¸*Ð?–SQ÷ó4ä?uÝok´?€ E eD?ì€lßYç?´{
?º«+4ÐU?³ûšŽÃiá?'+V!·/É?~ä"î3äœ?ë<Ô«³Øð?¦Mi³»®@?ÀçBŒù¶H?¤É>©£z?©(Oþß?R2I{D:?ÖË?Ý²")Õ5?Š};$ï½?Ñ4¥òŸ4FGL J1827.6-0849¿íÁ©œWJP?ótx]ï"À8E`؇ëòÀ:¶6eÃ@s¶0(@¼>	P?´A? ¸m€?ǸTÝ¡±@ÿ¿ž ß?óôÃ¿ÒçƒÝD¿?ïðÏ@D"®¿ä¶ÉöX·Q¿ä±F^‰"¿ë:¢hJA¿æ"ÌàîÂÁPSRPSR3FGL J1827.6-0846PSR J1827-0849?Ÿÿoû>2P?"
^	XΨ?ÜF'R| ?ÆðfnՓ¯?àýá>üÐ?ÆÄzŽ§K?'Ðk\¾ÿÁ?Œ$öbæá?àìåž*u?Íôí¢=
?ß/¢Ùݳ?ͽ†_ÐñW?¹æÖç]*Â?3}b쯩?ʜ<%¡€0?¬`R4׃?æ«úœ?®XVð-`?"¦W[2¯A?ka$1;?áU–•Îo?²†)ôrf?Ü°Žúͨ?²h]ٞ4FGL J1828.4-1059¿½œ¡izJ§?£1]<F,À7¯<Kà©#À9½Ñˆô/è@^Ä[@¸•";"+?½¡§Z!‰"?Å¡… eÑ@
2†!î?û§)Æwô¿ÜW'còà¿ÍÇNފd¿è.®è¿è‡B_ ¿ìŠ)º
­h¿â–¹‰$PSRPSRPSR J1828-1101?'¡âñwq?'Ââž4ñ?±,B+ÿc?µ…Ûwn?íEh¯ôY?·¾våæ?ŽìDLoT?"š4®g?Ìô^–½æ(?ŜՇôtë?èG7J3T¹?ÅzØ^Ý?·Açž7¡—?œrð?UhZ?Â=Z:x"?¤´ô÷p<?èˆl†ªm¨?¨>¿¢/1?rdcEaS?_|WYØbH?Áä­ôs!%?¥+ùÁ¤£.?ëb¼Xt›?¥O*Kª®4FGL J1831.5-0935¿ï¡ü"¿Œa?‰"ÏväýŠÀ7íèPïÝÀ9אíùm@Œú#G,å@@E]b×?ïd²Â4˜c?ÔEµV¬µ?ñÕ9eQh}?î%eJ´O¿Ëç‡Ù¿å4µê28¿îx8@8TZ¿ï|ŸB¥ìä¿ï÷8EÁ«1PSRPSRPSR J1831-0952?Ù½LµÛ*Q?Ó§Qœð?‡ÜYëÔ¢?¥M&–1¡?âÁégª»…?Òø—HÌÁ¢?±
nœ	VÐ?¹ŽG¤Œ?Õå‰se
?ÔFcDZvé?âëírÌ ?Ôcño‹)°?ÁÝÎCž¯?£Ï7á§þ?ÂTýǤ
?¢à¼vÎE?æóLýRë=?¬4cîýR?]>ìt5òà?nê*¡ÞP?â5¦¿5Ø??ٝÓ8¨ ?Ûws• ?ٔ›k·*_4FGL J1832.4-0847¿âˆqýã	?ÇÔeG'u'À8¡å$w¯À:áî¶+ ˜@ºÑ!Vî@U™Yعj?ÁѨi@5z?å×p>×V>@áµâ¥|&?ÿž5e§?ßî*Àr÷C?ãµ¾=gêu¿Þ5B,Oê¿á¾QtfÚ*¿íáv<?A¿ïÿè«î0PSRPSRPSR J1832-0836?Vþõøè[?SäÈ5Nt?í†ÛPIá?±vx‡=׉?³si¥ÍQ?±DŽ	Uãü?{{mTâ}9?"'Ñ;.?âÑ-·?Γ–ÑŠ
ª?ۆö¨PØÿ?Îlþ(÷?¤•cóá×?ŒqäX»?âþß/‡á$?¹Í¾w{À?×o•"tÕ?·¼¢^ØÂÍ?b¬n€ñÀI?Q]Á¤ü×j?èøØÄ>üì?²E¢¦"?ËÑë5EQ?² `Jd 4FGL J1833.0-3840¿àÕÞ"#…/À*€d©ÍÄÀ:¬îÐ,ӞÀ<£éå‡ó@Z­KR8Ý@5Êd{?ȽÊ{cÏ?à%ô»ÿ/@î­ÕÀ­@{!]æ–?ïã.qÊH?åòØ?ɵ¿Ýè{Vb¿ä Ï§Æ¿î‰›ár¿ïÿԖũÃPSRpsrPSR J1833-3840?Ðü؏Óm?ÁnÔw8Z?åYWV;…?ÄýÄqJbä?±AãQÒ%?¬\ÖÇØ«j?Ü£F(—È?Ë°•FAc?ÚAˆóf?Ëë2guÅË?°ðœêöT?»Ò¾WÃìë?Ö5E	ñEÊ?¶6›ßѳ8?ß,꒵†?¶Û¿"†î?Å; Æ³G`?£gpÚé=Æ?՞åò ?±óa) ß=?áBúç2@ñ?´øОª¿Û?¿l"b:-ñ?§ã6Y?Öv4FGL J1833.5-1033¿ìW'F¿ëù
ãˆÐôÀ79€C‡>MÀ:+-û»Í¡@—Э'Ñ@v¦ã.8"?§IÜÂ?˒Où<—`@ H,nóÓ¢?ñ¹Z¢
¢?ïúGߒ¢/¿ËYý¢W®=¿ä>ÚÑrMû¿ç
U=Ÿæ¿ë
+ãðU¿ç_QŸ/ÐPSRPSR3FGL J1833.5-1033PSR J1833-1034?Ž1W/?§VdåêÝÏ?Ù}-Äèæ	?Í#V¦d3M?âÈ£¿JÐ÷?ÍéÙǸ?uÿÏéR£?=b›½®?è´æƒ>Û?Æ{¡8ŒVZ?Îõ-í˹þ?ÆQ´'c
Z?¦óQ40?‰lAót?Ö[
¼ü-?¸4•bD¯?ãr1IŒn¦?·¦ò·É?,'ýé¥(á?­dNÞ¡?çbx‰•ï?°ÙYH{*+?Ñ8l¯/Ÿ~?°ÖÐ2èE4FGL J1836.2+5925?ãŒÛ@­ð@9(€QÉ÷À53¡Qô¿ZÀ:}àÖo
@ºMϖ«©?þ$Ã9¦?X±ÊåWb[?Ù=¤¦=@_jcÇOµ@)."?½ÒfÛ)1¿ÀËFý¿Ûοì¹ñ¿åùèÄzô¿î¯Úê¿ïÿülòPSRPSR3FGL J1836.2+5925PSR J1836+5925?[»>Ö<G?\´,'½?ï­&¨'õ?‰…Ék
°£?>ò8{j?‡ªIß­'¼?lH»•ÐGÐ?•äÖ¼:?î ¾"Ee?½‡½"˜?¤/"n¥?Áý$ó"Ðà?'[x@qØÅ?Š/ļåµ?íæÅâÖ?œ'/"O¸?³qëÀÒ£?—t_º†íò;3Í(†)A;p
©ýljã?ïÿä&r"u?ØzÊo>ëٍl‰@_?ØzÊm4FGL J1837.8-0604?åBQœ/î?Í2¦ÆRàÀ7èȼœÓáÀ9¬DmŒË@ W\ÆT¡@öÙæÃ1?Áþ‡ÚÕN?Á8SX—›¾@t#¾K)Ê?ÿý`Îvðø¿åÒJO¯j¼¿Ö™5{aö¿à×:yx'â¿èRœðf/	¿è»°DÖɦ¿ë"^~»qÜPSRPSR3FGL J1837.9-0607PSR J1837-0604?x&3ë®?së),Ñ×?z´ó <BÊ?"ª\DúÛ?ïšcÌW°?‰gC
S3?U\û«U?–9Êý'?¯Z¨øªµ?²ñ\j¤R?íƒm˜?û?´°aX~µû?²%ß-ø5[?—%D ró?·â]qø´?¡–¬È0+Y?ê¾øyrº=?¤ÙP³5Ä`?zvœ³ì?luo¶‹Ì?˜ç¬o«fQ?†woO¦†?kkd?ˆ6i›bc¡4FGL J1838.9-0537?Èï7t¥2?ÉzH†µˆÀ6é]…UÀ9¤ßI® @ lëT¢C·@÷é¾u5?­%Åask?Õæ͓œ*@'ڎO¹{·?î}Ððóȏ?ïh—c^t*¿Ý¤¯!k4¬¿árÞyzпãORúȉ¿ëÖWûi˜J¿íCèWlÎ_PSRPSR3FGL J1838.9-0537PSR J1838-0537?rʃe0¢?ÊIUØE?åLÙà~?ÎR€ŠàO?Óô;@ëù?Ìt'™™Ý?i.¹x+Ì?t…¤¬ï°l?çü—Fl‰Š?Ǧ£_€tB?Ϩèm-q?ǜ"sÓúÃ?'ºLIá?ˆ	Z–×ñ?çEÛwg?¶wZ+GÍ?Ðá8§|m[?¶+$À³©²>ӈþVÿµ¦>Ê¿Î0Ð?éתQüÃ?±ŠÒëo|Ð?È¡/¦2õ?±ŠÄ_êy4FGL J1843.7-1114¿ïót6¼2SÀW=
§ˆÀ8Œ»*ƒÀ:ꨆœfÓ@³¸ʏ@FKùӖ?²Àßٙå?Ô]+ß×Ár@¼ó…@=rŸ.ÙÝ?ïÿºà¼ô¿ÛUçÞK$l¿ç™aOü¿è®¯?ôÖ¿ïÿûÎBÓ?ïü>>ÿðPSRPSR3FGL J1843.6-1114PSR J1843-1113?ÎzÎð Où?Þhbwžm?ÜٖŠ¸EY?ÈãNl˜ú?Óéü÷'¬?čXK˟á?±®¼¯!k?¶¡mÄÐëã?Û,š¨Ì]?Í׀,Þ%?à3Ûµ£Ô?ΡMR	m?ÁŸA××Ãù?¦f'íÀ`©?â
+¦Mê?²âOÏ[?ÓÇxIÈ?­Øû|Û?¦È?J@i?ŒÏ뗒û
?ÕñÖâ.¿F?·ÞI06:Z?ã¦
óüV?·ÁÒfå3x4FGL J1844.4-0345¿ëÆTx'Y
¿ÅDÜþÉBÀ7ˍ¶6ˆRÀ:|TŠ›ÏÕ@ùà×Ù@ÌÕeø']?µ¬]–‰î?äï »ç¢@&W?·¥ô@8g'›%¿ïîB_Ëí?ï[Á&¦\ö¿ØÝ>|¿æàzÉʹͿî»ûXÑRn¿ïÿl\I¬òPSRPSR3FGL J1844.3-0344PSR J1844-0346?+bVìƒ?ƒÌ"3Vú?ïf3+à?'¨Ú@âž?…Rœ]"«?‡™ÌWîB‡?tAeUR[?~úß@ŽÑ'?ꅾJ¼
Ô?Á»O¸ÅY.?ÅFþÉå?ÁŸ­ÓýZ(?›÷u,wSç?¯Š¯5ß%?êxªè!Åå?«ùæ'?že¹éýï?ª_|5?4"ûM›ß?%!N­Â?ë×i;ë^?§ÞÜ¿g?À˜¦«»?§ÖĀþú4FGL J1846.3+0919¿ï¢¯º9Ĕ@jš^»w:À8‹ÛYÀ;¦1Wà@˜–t¸@xs€?£×r࣢?à¸põ5¢@2Ôm?ž{@¤ŠM÷.Ë?Ëìւƒ(¿ÉîNý"õ¿Õà3œd¥¿â¹q:Õ¾ä¿îD žq¿ïÿlÞfþPSRPSR3FGL J1846.3+0919PSR J1846+0919?f/³íK¸?jîùà¨?ï«Fs›Ç¯?…"Ý ÿ¯?Dìq%'¥?€Öšï%ïr?y:wÌ?‹±oéš?ëÞýŒ5Q?Ųä`-í‰?¿~Är¦äò?ÅD™£qƒ?£aöÜI7œ?™¯w,r
?ìtºh;‡? ]/n)m•?²©1Qy‡ù?"À'¡]?>—>·q?¸'!´?ïK];ß?ˆ´'¶?–†9{ÒßÌ?‡ýüƒÛwT4FGL J1852.2-1309¿èÀi´qÀ"ý>" 
À:#º
RiYÀ<'@ÿ¥@žD 
é?ÿb‰,d?Æõì€Ç:½?à=òÿf}@{ùiãÉ@\u'ŸVG?ïö.Åæ(¾¿»òªÝ¿ÔH$ÜÙ4¿âg$ÒG`¿ïw^3'þ¿ïþº…¢kÐPSRpsrPSR J1852-13?¯î/Q?¢W倬Ó?á¶L0ÔÙI?ŧÛ>d5?ؕ¤^PcL?Āûî◶?»µßU."?µû·ûŒúÜ?ÊXÆ1¤?Åc¬f]/ž?åóˆñ.}?Ç¡Ô!
5—?ÁSÃÙ$€?¥.ÊÌێ?ã³.É%ƒh?³øœì›õ?ÏàDÍã?¬hÕý¬ó?ÎûX8Ug?£ŠÃo¢°?ՌÃXvæ?²'
¾qâ?ÚõÞ|Ց?¯½"û]4FGL J1853.3-0005¿¶¨FŽ¥aÞ¿Þz5›mYJÀ9 òxXrÀ;"!\q@ "Dû݆ƒ@–ÖZ²Ô?ÐoÜ†©'?çFz7Ԃ¤@Íÿàè@g ÎN¿ïÿõEq#?ïÿÙÔóü¿¼¸j•6|¿ÚÌaÿÏ¿ë3g5™?¿ïûÓ {‹PSRPSR3FGL J1853.2+0006PSR J1853-0004?¡Ä\1>"d?˜scÒ2¯?ɧô!~	&?¸©/?ù5?èy½4Œ•q?ÃÃé½dÙ?™ê¨]à¸?œú¼Ÿë¸?×?/íŽÍ?ÐC£oÑך?ã'ÆIûT?Ï×à	½?ȒìÇù?¦l¨(ã6ä?Éøù?§U{'ÊÊ?ã›8†m¾?®AFÐßȪ?°-©ªa0?™|[ޓ§?㺇ð0?º¢Š¨º­?Ô‡¦©‡T?¹Vv'¥³4FGL J1855.9-1435?¥¯Â¾À•hÀS# îøqÀ9ò".E©À;Ѿâ(~¤@€ô2}@3•#SÀ?¿.æâšœ?ÆӘ•±ƒ@®p:û~'?ýQ§Ù"q?ïöÅúJ´Y?薘ȹAÖ¿âê¹çíºƒ¿ÕÜH)¿ìD~‡Å\¿ïÿ*¸:n'PSRPSRPSR J1855-1436?ß\o'B‡©?ÀÀð]üa?½ž5¬Ù¨v?²GpyÌ«w?Ù<‡9?À¿{"aœß?Òpà¡4K?Èzñ$
P•?¶Û\'D#
?¹Gb?ã쐊Æáy?ÉÙp#q0?âgƒŽùÖ?­©v'-+?»5V}Üwù? è	CçŒ?ÔdyYjîU?ª-Ceiž?Ö=
€ŒV?®¯>ò»Fð?ÒúÑ9S‰?´&Іãr0?ÖÈÔF  ?°w²5~ü4FGL J1857.2+0941¿ÆðE=ÝíB@ñ|ƒ^À9B%ÁZ¨ÃÀ:àãܳʝ@=ø9âû@þ¥2?Ë°›=އà?Òõv¤¢X@÷Eî Ú@½"ñÙÍ?￶Ï4†¿ÜœiÌ2ô¿é3Î~}´a¿êæÿQ"W¿ì4q ԋ޿ïúFsBîPSRpsrPSR J1857+0943?ÕƆêUÙ?À'ÿqZz?¿n-u%|?ÀLŧ°š?á.öÜd?Ãî¶øNÂ/?À³ûü¸?¸3ŽóG\¸?π ~ç°?Ä{>–yó¡?äJáG
?Æ- -ØQ?Çò7º8B\?¤öáˆ}´?ÂÚ7Z呶?£CÍ"2B·?åLä:¸Šû?¬€'¸C³ú?ª	¢Tw¸?Š¸ˆU«?ÌðnÔ³¶¼?©øï>.?ç#T­ÊÕ?¨Ó­@£Ë4FGL J1857.6+0143¿éü%kc?¿âÓ_XU+«À9ÐQ¼‹6À; B\›âI@ ìÓRwò@'ß­*p?Í@zï_t?ïÿ¤€RuÄ@r²žM]?ÿäP\8åû¿ãú=‰Mq?ë÷u¢™r'¿ÙÓ7º¿åq"ý€Hæ¿ð?ïÌ+òÍ–PSRPSRPSR J1857+0143	?˜ê귀ݳ?½~ÀºüùP?ë"ÏáGT¤?Œ¯'BŽ¦?½žÆGå#q?Àèä°Wñ*?‰(Xøí?–}±Ó[N&?äáÃ>À?ЅÖJôîX?×6£t¸¹°?ÐI_Œ!¤?±à…9
?–Z!ò??á=•Xn?³myþȅù?ÙBÌ.tã?²
Ìmw?Pjµ&àlî?Eч6(A?ì—Ä só?°-<•Älñ?»·`Þ³?°G Çx84FGL J1858.3-2216?àÙ҇nSÀ&ÉE•5†ËÀ96$)ªô5À<.wîN&Õ@÷ýÙµœ@ɪ`':P?²»dš‰X¯?ä:¾ÖêÞ@)¦XĽ4?ú¶ÛʚC?ïî"ã)/¤?Åvpõ‹‡Þ¿ÐYÏêŽ~³¿æØßT¹Á¿î @gNC¿ïþY¢2ÅOPSRPSR3FGL J1858.2-2215PSR J1858-2216?ýpGT?LŸò;?îN"›1 \?³UÅêÜQÖ?¦—Z))h^?°}YéPË?†rÁ];Ç?>š.iì‡?í»i3`³;?±ŽsÂyïˆ?®¬å™}O?°DM8aLš?'&ž²†t?w®½rŽ˜?ìì"Ì%‹?—ñÂ1w?´QÕ÷º2?•‡PÜåî½?.<Ÿ«sªÛ?è‰{C@ç?oY¬ç?~–(‹ù‡?‹Ýqªæ÷Œ?~n+XÓ4FGL J1901.4-0126?È]qkÊvÀ¥úÐìÀ8©@GDbÀ;Ðzw@ c°(§>@™,d?°6{<6g?Ôz …2`@µGZ1¤¾@ƒG#€Ö?ìÀÂ}h‹…¿Ìo`¥aÏ¿àÛ¸•Ò¿å#'†Wv¿ëò"a¤	à¿ïÿÿ&¦³PSRPSR3FGL J1901.5-0126PSR J1901-0125?ˆð‹Øƒ0Õ?€:ÞzHY?ê±(ñŽ?¹#Ä¡«?ìS~=V¸?·óB0äË?›˜	@ùH?²3hÔد?ãX'VR7?Ê* –÷>?וZ¿Z'ý?É^5çÏ·?•&Ñ Ã%3?ˆ<i)ü?ël3©£´ß?¥×ˆåº÷5?¿T®J±¼?¢ò›ÏäÐ?¡¦Ô¸±ë?|"ѐR?ÞÖÛáLæv?¯¡-c³b?ÞôI‡œéM?¯ÊÕý1š4FGL J1902.0-5105?ïâÿýYe*À6`Yž×ÇÀ8'hŒ±SËÀ;¯ð†nD@óœR†Šž@1¸YxAZ?¤—XP µ?ÑòñCú€º@(·×<'W†?ÿQK¯€á'?ìô'ßíæοÔíï\C͵¿ãÕ¥ÿ-¿æÌ£FÁ…q¿îß5/7¿ïýG¾Ûr'PSRPSR3FGL J1902.0-5107PSR J1902-5105?žu	Yò?™7–f?ìþ ïö?³ñ™šP)?°rŒ(¢È?­ŒÐ™ø—J?–Yô÷q×?™ˆ›d‡(Ï?íÇÈ
ƒ¾?­qæ-ؖ?¨V…#l7?¨.¦1ðèÚ?°
E'–À‹?€‹¤D­@?éÌ°¥õC?©ßÉï?ÀÈŸ`~³?£X9ú¡õI?`Ƨ²\ê'?Rˆ~•>Ý?íüÝ"¾n?—¼ÚºH+?¯%Ē®J'?—|ÃPòçš4FGL J1903.4-7053¿æÚ?¯îÀ:~¦Á HàÀ9øy5v'À<ºø6#@ŠøEÌgø?þ{9wÑ?·>,á_€ï?ã'Èâ\@!$¢v·í?ÿnãMß¿ëj2±‹(¿Å¸À¦MÝ¿ÁîŒe(£¸¿àfN²Š¿í™ÀÀú܀¿ïøÆ+$qPSRPSR3FGL J1903.6-7052PSR J1903-7051?•Ók¼m.'?™1<xĄ?ïÁfóv? Χ$—<?{QþQŠU?…H*»PB1?œðý[x@º?™ª®˜ ¢&?í‰,?±TŽ8ØQI?°"ЄÙ6m?­ej±N?¦¾½¬Ðçå?—fü¿øvô?ìLs?L¿?ŸN͓L	?²=/6þ?'åQiu?Ÿ¾7߀Ö?‹AYê"?ìwšÇmĶ?¦Öñ×x?´S›Ì±¤Ñ?¢›oRîˆ4FGL J1904.4-1129?à]´‡l׀À $Ï®ÿ\lÀ:ÇnìFå˜À<dÍßòC@}ÂuÛÏI@£°#HÚd?֋Óyq?ãRE|áÒî@~zÄÂ<P@¾ÒEå?åŠ)ýýÇ¿ì&á`'¡°¿Ôöǝ
"¿è€ôËۿïÿþó…õ?ïöÔþIœPSRpsrPSR J1904-11?Ñr}7?¯¹»j1p? (º(+q¾?™c57Ý¿?æDrò	I?Ã5
@?Ñé?Ø'Eh8?̒'òÊî?"ÁŒ×ÂPõ?œ9˜Tõä?ãNföÞ]?Ì&wžíNž?ál4FŠ¤A?¯d&s†ø˜?¾0òÇ(s/?šÿ%Òe€ ?՛ZÁ š±?¬
 æÙ°?Þ§p,@|.?µl.‡±Ñ¡?¨ç†Ì#£O?"ÁL¨çJ?Þ;žú;h?µ*KBÈOP4FGL J1906.4+0723¿í²ê\™wÐ?¬)¹úµÀ7Gg"s—§À9ÝZ±&~@ÔŽþ
2@%¸ m]Ñ?°Â÷Æ´?ҘnáµD@%Ԗ$š@°6ú*O¿ïcÔ?ïø{§@KJ¿å4>vn¿æº¯ßV¿ì£¶ôs®¿ïÿ#+~3PSRPSRPSR J1906+0722?'ý'}fï:?º…cô÷¶?핒q;õ+?ÀbR'Õn?­(­5º?´{ÅÀÛ!?lüÙ§ä¾?vO³Œo2¢?è›&"5?ȱ™{>y?Ï ‹˜?ȨVym4?¡nò¼02…?'PZ'áP?â+¬ƒSRÅ?¸P¢ˆA?ÙzÈ¡ÓT&?·ÚÛù¢þÔ?¶`iV‡?›	E^ñ?çi@B-ë?·þ"(àÝ?Ñ+"£ÂL?·ü¢äwõ4FGL J1907.9+0602¿éO'X8¿ìÔpÄÜ>À5äÜÊpÑúÀ9¾ÕöA:]@€Î(™Ò@Y9W9£?€×@ÕCz?Ó
Žÿä:@?Ÿ‡ð#ê@A‰Km¼œ?ïìu¿I×e¿Ô€ä+Ž#D¿áú@m®YD¿åÒdáÖõ¿ìøb²|¿n¿íãP!U*PSRPSR3FGL J1907.9+0602PSR J1907+0602?4žfó¢"?/½÷oo±?ïBj¹>ƒ=?–Hãr_ù=?—`0b"ÉÛ?–,¶-¹Yš?[¯Þ\nF|?t»¢ …T?î¿ÀHº?©d=•L0?£2uìl?©ÿ¥£‰Ý?~œÎ¥kÄ.?qV¥Áu\?ìIāŸ?£«ˆïa›Š?¾äñœ¾È?¢øÓ栖ì>KÇUÚj>]\®ÚgŒµ?ïÓ¾(Ûó?–¬À
'?…‡\©ÒÛ?–¬¿²óü4FGL J1908.9+2103¿îåЛ®$@è^ùŠ›À:7ÉÞÛÃÀ<Ó;{×@ÓÇ­©@±¢|—*T?ÄïL>h?Ü¢)` §@ö=Ÿ@Afl›‰´¿Àôš	¿çù5
¤¿«lи¿¤›¿åLx~–ÞÔ¿êáfµN+¿ïÓ	'Où=PSRPSRPSR J1908+2105?¥W†ù3øÁ?ž%°eS?͹8ðƒòÃ?ÁG¥™µñ?ç<9TKÃÃ?Á°Éá-®J?Çӂhoî?¼áŜ5š'?ÁŸò—Õi[?»0	²;7?å£"¿îàn?Áê÷ðÓ¡{?ÒX¬Ö{üò?°S:÷ÁXF?֜sˆ
?´&$	^Ä?×
ß¡vï?¯/¢e£(?ÒaŒŽ'?§4Kóþ$÷?Ä«yêÇÑ.?©Þ"~®e•?áÓñÄj?®²~"Y`4FGL J1913.3+0905?ì˜ÖI3‹Ú¿åñ|‰'öÀ8¯YAºµÀ;0Ž=E@d"iS֗@ñÓíR~?À÷ß`"U?á
&"¿?F@¿b€þ˜@³8•¶Š?îœ"_ü?¿çædžJ ¿Ý %ú»r‡¿äÑiêe¿ïÿôÂ_5›?ï÷ŞÛ!úPSRPSR3FGL J1913.0+0910PSR J1913+0904?ƒNï?›£ð˜i?îïʗðz?²°ãM;ã?˜_l2ù5¦?­Œúqtˆô?'kÎp*Ì?'Ð%ݞ?ãm›?Îø– Š"-?ØóÝN?Îl4VØó?¢ØÆ qÍx?µÉ¯'?çÇMWíØ?±—Ö(¤?Ï>±"ƒÕB?°<Õ6aKü?s~"–q=?c«+î*oÙ?æñkSFx{?»Tu.ÄÙW?ÑÏ/S`µG?»pø!ã4FGL J1913.3+1019?éÏÑm+¸§¿½÷'qøÀ8º(8-m÷À:gþ¬Bê@!¡žJÙB@& }¹i?Â6F¸÷?²n·Ù»s?ù…õB6Ü5@*ívæfQ¿ß`nŸðË°?ïò´BgXª¿×
¼;Ú÷ˆ¿å ø0'æ¿à®2ã'ø¿ç.uÉ°¸šPSRPSR1FGL J1913.7+1007cPSR J1913+1011?¦˜v÷J^?Ÿ&õoÆ/?uÿ]mÌÇë?x3
ø%
5?îjyÕ³Ê? ÉÜ0î?³½!»TöÏ?²°e€
?€©m™œÜÊ?X(ÅèxÛ?íE¶.í´?³ý÷\ÕûA?¾Xk¢Ä?¡…çqGå?¬+¼¯#Cå?üÞ½ ?êrC3 Wi?£eÑľ'?»ñ"D9êM?¡H䑒&l?šÏGØ´?…ê닧?ë«Q>ƒð?¢ì=°¡O&4FGL J1919.1+2354?ç¦ÚðQ`@å9û¤P­À:µflE£xÀ<Š˜¨ØѾ@ÏÓ)`G@ãŸý`éO?ҀóûØÑ?ïü³åu:?@_–ž<–‰@£º	P¶§¿î«rßñm¿ÝiÚ¤¦½ï?ÞUIž¶™¿ì²ZÆ3¢¿æ¶õ׈¿ïÿѧ' ÖPSRpsrPSR J1919+23?Ãx|Pœ‡?¸œ"÷Ñ¢"?Ð[bðG½…?ŕ7Ÿʨ?âôNhÇú?Çù'§Èf?º «h½‡?ºÌ`è•HÛ?Úæ3Óè?Ðû.¥N?Þr"ÎQè?Ì]…|¿ç?Ö'›ê"e?³Á4̉~·?ÙúçÂ7ç½?¶j•	zH?Ϻø¦h½?§6õY=£?øQ¨ÁáÕ?²RûIºûâ?åÃ?Ñü4?Áiïîs–?È(¡Wö-]?¹R—öL¡4FGL J1921.1+1930¿ïO¡L…-–@ÃA2Ð7À:YP¦á€¹À;Ù'æ÷ñ@ 
Ž?w4@Ã/M= ?ÑcꠝCó?â©þk«@~Ó½Ö.@̸
Íóé¿à™æõlÿ¿èž÷ýR%½¿ÛõÀ¥Í¿ÞVe9q'¿íM,Ù|Þ¿êÔÁÔiPSRPSR3FGL J1921.6+1934PSR J1921+1929?¥9ÊÀt©Ï?™þ4óé_µ?ÜÂÞèRÑT?È7·ˆÝ?àJóßÏL¸?Ǥ¶T?·eª‡~û?µ._øÄÑ ?ƾŠ¡\Ê?ÂÆúpü•o?çc¼BXî?ĺs¢Þ€I?Ó'^à³æW?«¨>Æix?щ²çä#?°žš0šÌ%?ÛNîd5…?¯o¢Ð?¸s©bâ ?Ÿß–nil ?ÎX£QÎ'?¸'7šN.b?å[aÿ0?ºhíFu,4FGL J1921.4+0136?ïÕjT 'pÀ·rÁ¾{ÑÀ98èÑQ­À;Ù¥J_ @"ãð)ô@÷¨»uŒt?µ™ËÍ]÷?Òù,Ü×ÜË@M;ÞÓ_Ž@×£—'?堟²¸N'¿Þµý½ÛmO¿ßîÝBæ¯w¿ã¡¸LH
¿ë`0âvd¿ïï\ÏõPSRPSR3FGL J1921.2+0136PSR J1921+0137?žòJ*ÔSz?šxËyPªZ?ëí[Uàá?µ2ØÖ~?¸Öꚛä?±œè[ì°x?¤D:±›u?¦6HÝÓ?䷟eÝh_?ȦM<;¡Š?Ô9Þ;Ö?ÇkÐÏê†|?º9l!éhR?£z5Tn?å弌?îx?²'9²‡?ËLW¾'ò?«,OUvm?µŸ*Ã(;}?'ô³è¢±ˆ?æVB(sÅN?®ÿÐ"̍?Ë×aüœÍ?¬¤ì	Q•M4FGL J1925.2+1729¿Ûâðåk?æ'ÛçlÀ9ah¼O§À;:²<þŽ@(QغÂ@Ût´?Ê]?5Êè?ä"ûmI@9!ßyx@ÕäÎvE¿ÛxH[c}ÿ¿âÄôÉ_¿á5^Pp¿èõPPx¿í‰"Ô7û¿ïÿþó…õPSRPSR3FGL J1925.4+1727PSR J1925+1720?š¯ìZ^ԋ?ŸæZÊy?ážÄ±Á?È7»Îß1‰?Ûy&¯5?ǜ.©Ü§ ?Š«"_C?ªtÿt?ÇóíÅ$æ?Âw¥­æ'e?隕â3…J?"˜Håúª?µ¥âHn	û?"á
à8—k?Ö\Ožb‡?´žE'lk?â>#
~?³Ùµ&â?zãAÒ0ƒY?e¶»	*†?âßÀæӒ?¿QOÌ?ÙÔñ+À?¾è6ÈÃßu4FGL J1932.2+2221?æ&zÇ,µý?ùYº`úÀ9ÄN`	UÀ;s'È@½S¸cß#@Hæ=·´?Ó=`]¸Ã?ۉQÐ9¿@M}|,¡I@š@Zãü>?îÑÇ]w)'?ïý¶ÿÛíÒ¿â—DŸí˿刘ö«;¿ïܤ`œøÊ¿ïù¿tµÎPSRPSRPSR J1932+2220?ÍêB€*Û?¼õÀX»è§?Â0D~~?¹®3v¬¿?ä79^@UÉ?ÂÜîFv¿?´Ps7æg¥?ºãÌ+Çÿd?Ã>Òßò?ÃØiõuºƒ?è¦mdK6"?ÈU%-Cç?ÁS	
øû?œ‰J³­¤Ç?Å;tœX"?¢'²»'Ó?æ\`¶Zå7?¦ó·¢ÄLè?³:ُ[©?•Æ`",@á?Í5Þ;Ôîš?µªÕÆ;?æK-?O9?µ:֝)NJ4FGL J1932.3+1916¿ÔœE~lö?µb©ëJÀ7~ÔÈCÑÀ:Ž•yy@•ŠÀÏ6@¬Ÿ€cg®?¨'¼«ë¬?ÛUߛªd@-ïÓh'1@>—û^ۃ?ɍQâ É¿ÐB3µ¿âé¤ÿ~Oç¿èÛӀE4½¿îf«esø¿è*AA¾¼>PSRPSR3FGL J1932.2+1916PSR J1932+1916?SàšHW­?Q'Wøë¸|?ï0ã±.1]?—•4ÌeH±?˜¥€8eNÊ?–Åâ)PùT?pbIF[?ydF¨(¶	?ëJÈçSf?¸´ÞêPn2?ÂQÊ9…š?¸-3‡¯ö?‰K×ÄÃ?qùÉxÄA~?ì÷4étþ?¡ç•º9H?¼VË`3ߟ? À"KàÄð>ù®L£ÉD>ñ@U§3µÓ?íÞôÌ<¸ø?šìì÷™?±¾´En?šà®Ó5•4FGL J1935.2+2029?ì6{Fi¾,?°¼ÿ¿KôÀ8fpȍ£À:~E܃#6@Ú	Òg@±áYKË°?½(Eëf?ØPø€"Ê«@"³Ïà@{έw?Ôy$ä»ÖÛ¿ØH€aå"Y¿å¬:†
˛¿ì!ùOÖοïÿþÐñ¿ëÈ:a$ÞPSRPSR1FGL J1934.9+2031cPSR J1935+2025?ã
€
?˝ªÜ°Îˆ?×ãi^5.§?Ë®î‰?žGÉì«q¸?žµ¿½3T{? €'ƒL×?©V'í¹R'?Úw3"Z?Ïígÿ‡¡?á¼w
ž%?ϹۤÚt?Ë*ü~‡)?±IõyŒ³;?ߨlõ4ÀZ?·¿øõŠÆû?Ò'Œ‹ü?²ˆå+}ê?6dÜ()Ñ?wK!©4ˆ'?۔@ëSv¨?ºº"R|?á¹öå¤?¹ØØ(sE,4FGL J1939.6+2135?âo'EM£¿ÒÚ
ã]Ý×À8â5~gÀ:Õoê›ë@.|Ì.lO@§ B•¦Æ?¿æ"´4û_?Új{ßI| @°lÊ-¶@Žg£'aï?ï²;†¾Ë'?׈Šþv=¿ã"~aÚ»x¿ç«Œ‹¿îŸ[O7¿ïÿý¡UûŠPSRPSRPSR J1939+2134?€©DX'ö?}ë´H/?îÚ£œ'?¡ÃN•#Ò6?œœÉ
Q"Š?ŸŽ;øEK5?ŠoaȂ'?a¾ß%Ü8?ᘏfÂ5ù?Å­œ¥3¥?ÛûhÏmOù?Ŕ=±'K?¿ÐÌtç0?†1Oòìÿq?èuÉõɪ?²@Iòq?ÊpÞò<v?°|üÎôÄt?t[éÿ>?[Ó¯‰]±?å!\<æQ?°L´Uù?ÕkÛ2»a?¯ð7Õ׎4FGL J1946.5-5402¿»@ˆñ«©gÀ='…¹èÄzÀ9q0ž-}À<§'ÍÍ}Í@-µ"2@5¦à©ùc?°x±'ž‡?âÄ ¾{ü%@(ÐkYnL?ö	¸éžÀ?ìÔ þþ"Z¿Ôÿž[JT¿Ô·ºÁÝZ¿é‰²€ñ,(¿ïÿ«çy÷=¿êO]ë­¹PSRPSR3FGL J1946.4-5403PSR J1946-5403
?ŽÞ1àQ2?ßkä>ÞP?ïmCqJ÷?°'´¿sDó?Æ}C\.Ü?®ÇA·2yJ?"".."»R?—0ç0þ§?íe&8tY?µ`;9
?¯œ…_÷\º?³Ížn"p?œV¸Àû5?‰b{»È'Á?ì8Â!7¢g?¶³ãE¡5?·$@ó­ú?™ƒ}'¤²Ì?%ÏanCÝÿ?¯zÆwŒ?ïÉ.×Q¿?uùçÔ[Xœ?zºfå!?uñ`á¹[\4FGL J1950.6+2416¿Ãþ`KLã¿ò[vH[¹À9Z`,ÃÀ:Ño™\@ˆªFJ@Á¹Þ³?Êuú	?Ðеd¦GÓ@
¸S 8"¬@øᬭÈ{¿êÓà뽩?ïÿ$m'M¿ç`Jù"–-¿çÛ?áíEh¿ïüäW-
¿èü{±QFDPSRpsrPSR J1950+2414?ÇÂzX…Ü?Á=ããϚÝ?£Wđz+?Á¤Ý?èÙå à´¶?ÁùeQ¾~"?¶Û̌R|À?°úï™(?°ðD›r¦þ?¯üÃi¼Ðe?ë}Û[‰?µ³:Ã
{?Â8U	slÄ? É"kQ2?ÀÕ«x˜¾§?ž"|ø>?ç<ß|õ%?§K÷i©†¢?¹LfÝ"È?›ïmÐ¥ù?Ž4ýÜí4?§Š¾Ä·Þ?è2åää"z?­å!áSF4FGL J1952.9+3252?î!?ŸlQ@"™Iè^À6¨V˾°À:¤NA¬rº@G¾"¤9@a59°€?'	ÉSØ?ÑÏrä¤@<¤Y!…Æ?ü°ô9MS›?ꨏ òSo¿Ð"žry¿áÇggî%ã¿å¢l ºŠ«¿íB XÐ{®¿ì†XVÙ+PSRPSR3FGL J1952.9+3253PSR J1952+3252?R­D"?SNiI¦1#?Ðô3>?¦+1d0N?¥C­ˆ$¡î?¥»eNÑö?d¸HdÜ
?zƁŽÖ–?î ˆÏŽ^?¶üsýßÓ,?¬«î‰5l[?¶¼L}PìK?Œ«Ì+',?CDÌJ"
?ë݂úµìA?¨ëL¼¯<?½~n˜K+²?¥Ú3^1€>ƒ'ó‡#5$>"òZËÈ	á?﫹RR{?~IçÄ×?…—É·Ùç?~3ÕÔ9Ä4FGL J1954.3+2836¿çî˜'Q?×â4½÷ÇÍÀ6òçø¢=­À:{(‹9"†@ODL
D§@‹Ÿ}ß(ð?œC¦·©?Ô¼íÇWæ@4ÉîEÃX°@àp©?ï÷uýÞÄ¿Ì¿¯î¿à²¿-¿åÛibš)¿ìhÄÓTÑ¿ínúSPSRPSR3FGL J1954.2+2836PSR J1954+2836?R¹~¸p"?Q©T1JI?îezÇ,6?©žŸá‹½š?©Š™Fڇ?©G4kz?m	¨8õÜ?vêg0õìˆ?ëŸtݧf.?½lÌ_†4f?Á
ØbÁƒv?½LñrXÎ?€­œüž,‰?i«"O?ìèLë+4?œ÷€9?¶§åš?šÌ@b"÷>ޅEíºF{>ãpP{ŒË?í¥üÑö5?žÅ­ö‡?²ÏŸbX—n?žÄªR*ä4FGL J1957.6+5033¿ï""mÌ@&	»j¤¹ˆÀ8eŒ«tqÀ;ϽƟŒ"@ýÁ@¸ýé¥K?¨®'zšÇ?威‡ª@5¤A»Œ2©?ý]!ŽpÅ?î݂AŽ?É¿ÌÝÐÀ¢G¿ãµJÐê°¿íP,h=Öû¿îÚG¿ïÿMéDÓPSRPSR3FGL J1957.7+5034PSR J1957+5033?UXûæÿo?ZڂìêF?ï}H"á¹?"FÏzõ]f?Ž¿J±Ñ?"&eOu?ƒ´±Ì´
?£J*Tb/°?îïuÙ	?ÀÓ"㲏?ªóÜ3ðBf?¾¨Ðß]Žƒ?¦Ð>/ÏÙP?™åÅ¡±Àƒ?êô«ïŽña?©kGär­?¼òk ˆ[?¢Š#ÉSÅÓ>ĶKÏê'>ȂØƹß?ïǯµDŽ`?s‰Dæßþ?|%Ž">îa?sˆCû¬°j4FGL J1958.7+2846¿ïâ6öƒ¡Ø¿ÖÚ
'ºÀ6ùgÉÉãÀ:—"rñ$@üi°ó¨Y@µ€e-?šþËD'?ÙoQ|I|¡@8‡Œ!áÒ?ÿd7È]?ïüÏ^w"œ¿ÄY€ú¼I¿àÁOÁs¿ç]*J¿ì£o÷à¿îBãÈÂýPSRPSR3FGL J1958.6+2845PSR J1958+2846?Q€ÛX"?VÇM¡¸®+?îfp·?®°~Án@?©Ñ5ÔW?®-"6ïßÃ?dÌNššd?rœZ¯z±9?íÅîwkÜ?°÷Œ¸Fn+?±,}â,Jú?°¢éjWs?³JÛ™ò?ráÂÜØ?ì¢GŠGþ?Ÿygl*R?¸·^xJŒÉ?žmWóXh>™—À´+S¡> ¯p'ê3?ï<—¦ëã?‹ñ¹ÉÆ{P?˜lñŠÂêû?‹ñ¦Sà'4FGL J1959.5+2048¿ì5	ƒó{ÀÄ{gkÀ8Ú·ÿ¶.%À;Àäù}@´šýqÛ:@›ì't¹æ?¯uÝöjÖ?Ü UàÝ%
@%u"BJ'k@•šw?ïÿíUÙPi¿ºÌZ¡Œ,I¿âTI˜ÐEþ¿çIÁ/à˜¿ï-ž§öT¿ðPSRPSR3FGL J1959.5+2047PSR J1959+2048?–'¾ÎFd?¡ãÁ¥L>?ì²Qõ#!Á?¶?‹7º]=?´ÈÀ£UXò?±ˆl™Òú?"½÷7nŠ?wío'Ì?ê[A¥!
<?Àn€#Ód?ÅGøâk?¿DU})å?˜ºfrc–'?ˆâù±?ë+<ÑHÎù?¥•  _g­?À;¿ìQJ?£µV¬¹C?cq'¨ÊŽ?P-ÏNà!ú?íÖy¸‰M?—Í]ð{š?°°¥¦q¡?—š|^b‡z4FGL J2006.2+3102?í^z£y¿á<Âþí±IÀ9?ô³›£_À;p.fDØ@ëÏtœ@¬¬Ñ"Âr?Á¡Èg7r?ÚÁl!'J@×Aü#Ò?Ý#Š'ÇpË¿ïþ2Œã(?ïòX½[jµ¿ßՁ;ÔÂe¿å+ùæ/t¿í"XŽÛP¿ðPSRPSRPSR J2006+3102?µ!íP	£?ĶMØ?ìq2{y=?Äëö3è3~?Qü{›ñË?œm'Š?}¦j‡Žt$?‡u(Ø­#?çänÖ0?ÊÅaݯ4?Ñ[yÜÎ?ÊocË)Ü?ªEš×»«ó?"Çtôß©?æ3ì³Ìï?´}÷=ö¾¿?Ð|äË ð£?²8ÜoSƒ?Y/Ðeár?F®ÁŸÜÚ?í½	U–±w?¡w®Mf ±?±²ö²î{?¡Pq­nÿ4FGL J2006.4+0147?êd'‡žÀ/ŒgœÇK"À:ŠsùÍÀ<¬é\OŒ/@Š"Yé«U?ÿ4?Žò?ědŸç¼g?Ú·u¢™r'@ª•…7âÅ?ï‹x~™?ïÊ\ô‰?·ºä—ï ¿ÍÂ\ÜNõÜ¿Ú¨ÓÞ¹ß4¿êÓÜ¡@B¿æg€)ÙîPSRPSR3FGL J2006.6+0150PSR J2006+0148?Üåsk_?ňdCTüê?Þ¦vdþK?Æc­.•?µŸ­&9?¬•£áŽ%Ý?ÆM±x€¹{?Éh÷@Kµ?æ¨Ê×N°ù?ÍLç]Y?¾FT‰9?»̳ã
?Óòæå©X§?´Ðè5¨w?à¥îŽ¾Òº?¶ƒÓ½™,?łwù²Ç?¥ªÝU$?¹våáÖf?™ýŎK?è&@r|ÔX?¬ß7]ê8?Â×BÃÃj?§‹4 é4FGL J2017.4+0602¿²{éw=Ô@À0Ÿb0vÀÀ8dÝÐ*OÀ;˜Å~ð¡@Ùtæ[ê?úក‰'\?¤ŽÁ¬æ±?ÚDãÿï9@5­¥¹bŒ½@/j¦¼î?ïÔ°á´»^¿ÁAá_¿ÌëõF";¿Ý¶0©7 ¿ëŠ÷0ÇÉ¿ðPSRPSR3FGL J2017.3+0602PSR J2017+0603?Ñö4	+6?…
µ]®`?ïxó÷HÛ?"÷GÈpë6?âI<×?‡îbL=̑?‹‹±KÁ•?'ÜIRil?îW¹vå±?¬m¥òC¹Z?£¬X¡?µ?©OÞ%ö¿ƒ?¢ÀX//Ãh?— o;?ëñ×­I®Þ?¢r¶°n?·~§]?›[5Ji?
#õ™j?šÉ¼n?%:ä1?—PíâjË?§>Ô¯
7?—â´¯44FGL J2017.7-1612¿ã<]©ÜæSÀ:4ÕÇGQÎÀ9ÎTæâ!ÉÀ<W^Æ^ô'@ˆ*Û Ð@䲁Çë¼?¸	{>d¿?ÑS•ÿ0LN@»Ÿ'x@mK–¬T\?ïê9>åîݿݒK|U;¿Ø¶<?@ˆ¿â•V©Zý¿íÂû'²ö¿änÒ ÷0ùPSRPSR3FGL J2017.6-1616PSR J2017-1614?É'š¶0N>?¹1ƒ%FÓ?åDu0y.?ÁÐÿ+sÑ?ÁƏ
Í
?´æj3ó¿?ÎÆ$¢e‰ï?à 5µ%D?âãfònö?ÉrãÿÛ~¯?Ŭ?"â66?º7ÛQÈ­/?ÎØNvLU?³% á½œq?áùÁt²?µ¤ø¯©?É@«¶é¦*?¥ y8ی]?ÔÏ!ā?¨Àt)Cœ?ÜK5dùµ}?°D×+¿ý+?ÍËQ­Ó?¨ØFžâE4FGL J2017.9+3625?äb1_7aÛ?Øç;x| À7`C{ÓÀ:l«,i—@Þ$ªÚ3¾@ªY:-ù8?¦ÐNƒèú¢?á߁ëR@1í_‹Î@¨¹(«?j•ExZ/¿ÚlªMF¿àPhb¿è¹¿èîú‰žyÓ¿ï4ör2M¿é"—VÉ:qPSRPSR3FGL J2017.9+3627PSR J2017+3625?[tèj«ž?`D5…Œ´ž?î§0GÚG?¬¾sÊQá?¤±Wx,þ?¬]š1&Ã?m€ÀƒûÒ?u¤ûÚ/
	?ê©ß;ðUm?¾Ñz7èÈ=?Äâ€.½ø?¾ƒÂô]¨?‹e›îÖÛl?yß÷Fà&†?ëFïe'Ûû?§ËÀŠ\‡<?Á-èªË"_?¦ÄEÀéü®>æyuäu>áÓßß´?îG .èu?—¬jñz¾?«Œ•ˆ8ja?—«gèç]Ë4FGL J2021.1+3651?ï‹Õg'?»ì˜ïû{À5^Ê÷àÀ9¿-<y-@îý­•O@âXýÈ[?…\¼!6?Ձòžm"×@J^$_ZÙj?ý|$C?ÞÔûD"i\¿Ða1ޟ](¿áLà«üÉ¿æW~6fÄZ¿íZhµËÿ¿îqžBuÆPSRPSR3FGL J2021.1+3651PSR J2021+3651?iýÀ]­?¤"Æ33ý¶?ïҚê<€?§J)ú¶ ?›%ô ºc?—ªüý	•?])Y?rËú>º'?ïu}°ÆÇz?žÐUpšÿ?Žûoë-aŠ?Zêv<ƒ?I}ïù!?y,ªn~?ìœð¡? G̹Q•¢?¸ï\—Œø²?žÑüC–='€":4> =Ç7Ô¥}¹Ž?ïòhn|™ô?eQwíI00?[/#´¥?eQwìMCd4FGL J2021.5+4026¿îuø#V‹@§~¼ž`À4æe×Ë-À9E¼Çœd@̧"W`9@èEc·_}?‰ñЁ&?Ù~†TB@Lôów[0@nÇ­Ô¿Ñ&s1P¿¸{w€Ñ1ò¿áÉ^ƒCÿ¿èU±|æ¿îÔvå9«¿îõ_þmXÉPSRPSR3FGL J2021.5+4026PSR J2021+4026?ž¼ü¡jÃ"?¬3µ©¬Í?î#Žßr}¹?¸€'Sðá?œÑ'pE…Ë?©ê!nÅ I?'•2oȱV?«å-Óü¿Å?íËÇIÕ$?Å]U´ôK?®ž>Æ»"?Ãʛ^íÜ?ÃßÚííð?°þì' ˜ó?âH`l¬;?´'ÓèFDà?ÑßЯ°?¹WàÑë‹=¶Ò#I‹Œ=ôŸÕg[:?ïÁo¦¦Úø?"×;E\fµ?H,«%bW?"×;C ]4FGL J2022.3+3840?¼UP©æ˜Ñ?î=oâ'JÀ8tPrßÀ:‰ƒùdo@8'l+w@i_?*¸?¾—R£/š?Ú8ªkxõ@©×ý'w>@,Á®
¿Í?îZná_+	¿â}]"ðÅпèrçÉ0`¿ç¹" ]îs¿ïÿë<ú\R?ïü›¦2ÚPSRPSR3FGL J2022.2+3840PSR J2022+3842?­
º+VB?±s{¾{M?ë±J2@`ß?¾V& "È?³îÑXoMì?´m"N®äv?¢YÔ¬r›?²ÅÕ4gç*?Ùàê©÷H?Îk"ð»?âr?ãã"?ÎY†zꅁ?»7ºn=«?¢¯ð€¡O|?áhÊ`Ó¨?´Ã£V%¾E?ÖaóÏ®íê?²qdJ!äã?¡×?ä?kbáèÂp4?ܨ<F¦!?º7·/¸?álž.~?¨?¹òæfÅú—4FGL J2028.3+3331¿ÜÞÒŒâÀ¤‡3eˆÀ7™ìløÀ;7ý˜F³@ļ YÒ@'ågÎE?¢1R»í4)?䪘Å^C'@8c^t)ž@úúr!…Œ¿è0SðBÛ?ÓÆìM›"F¿ÔôÃ@±öÞ¿çâP¢Yܕ¿î9Pƒ¦N¿ïÿþÞ÷PSRPSR3FGL J2028.3+3332PSR J2028+3332?3ì±g$Ï!?8«¹è©,?ïåKº•Ùe?p%ã_G|?h6¯=Bê?n;‹<âGÙ?pWŽ3G6ð?~¦ÏÌ?íQ)Ž"¿ü?¹C´ì»½ž?´q:¨¥Œ£?¸Ë7"0}½?"y®F{=?t××Æ-Ý?íhTª,ÆX?"9@÷õÒ?²+KxÐýÕ?'3OùiÁ¦>˜¦áDü>Äæálë?ïÏ]kt)à?q'¥‰P2?xPç­Ï‹Î?q'˜÷ %4FGL J2030.0+3641?çò¸áªÌ¿¿÷ ²BÀ7ìºç£À;EWøåZ@ÖâVÌÀc@Mø±W%?­Fk\?ãÛ'8S-¤@1-û¹@ÂC*8ä¿ïsÎ>º?ïþñ­VåÀ¿Ò@묋å¿å)µ/ê©¿íñ™ O–@¿ïÿý`éNäPSRPSR3FGL J2030.0+3642PSR J2030+3641?_Ph•ÝåH?a7¸¡ö÷?ï†ü2ÝPg?!ŒËØ?ŠVæ5ð)ž?Œz H¥ï?pג)r£?}Ž@FÆí?ìõóG¯³?µ¹]ThŠ`?·B줋X2?µDä{ýu?…ñ¯3"?v¨"ëb·?í5`p˜Ø£?—yñV™c?³£>ER؅?–›òOG?çcá àý>ü,Jº±;b?ïž™38?ˆÇBˆþfD?"9'¨nö?ˆÃÜÌ«Ä]4FGL J2030.9+4416?é1?Й@%z
XÀ7ßÉÇ^ÏÀ;(öýø¾Ã@Vv&LðÊ@Y ¡`7?ª'ýÀ'%?å-‡ÂÁ@0¨…<ƒE?û#H÷ë‰{¿Õ!ΜZ¿¿Õ{½ZéÛ{¿Ûúd_¦¿êŒY?¿ïùºá辿ïqÊG·N¶PSRPSR3FGL J2030.8+4416PSR J2030+4415?W†Of[õ?c¹˜yç9ÿ?ïhXžÏy?©)Fðb4Ð?'|‡-:j&?¨ÍÃyC¬?qÁ¯ŒÑ€ž?èËý8?êv–¼°"l?Æ.Ž'à‡?ŗ—×bK?ÆB-äœ?‡[`²EW?vY)yA?ì×-֛ð?˜r¨ø³'?¶\´×Ñ?––ûç€G>Õô¤§Ñ‡(>ÏÒ;½A?ï£Uä>…m?xŸüß¼i?‡'È[ɪ"?xžÕ9"õâ4FGL J2032.2+4127?¾Sòà «`?ðbá& %9À6ªŽÊ2¾™À:U»¹@ßuÚ!Ê?ÿ· ÈÍcÌ?žYÊC'?ØÄ6Ûß9a@7ÎáXu@7M­ÝÉI?èµólsÆ¡?££ä¡)ÛÇ¿ÕP<ÙO<¿àR©»OÌÇ¿ë†=Á×{R¿íIš³uòPSRPSR3FGL J2032.2+4126PSR J2032+4127?h­ñPLÜ?hã`Åqe?íƧ2j0?±3hF?¿?±Vâ,Â?°¥ƒåÂÈ?j"ë/¯¨m?x|¬«m?ëpñÖÀ?Ã5Å1ei?Ð,yæc?ùV7Ñ ?ž[p±b'?"«,ý;©?êr•Rݚi?©ÎÆj]¥>?Âs_Fsj?§G³J†>ЈäØêÎÈ>Ǘ_"©?íäCbýý¦? ñ&öÌ?°Ý¢Ä|¯0? Æ¦Ô64FGL J2035.0+3632?×BðØEðÀ»K›	bÀ9 ¨,"	À;Ý©Çå@'L
QÍ?þ°ð˜ƒïä?¹§µ\˜²?ê€ÖõD»@(WšÏú@ˆA¿ïÀ‡—ů?ïÿ胸›?¶Øíþ†êQ¿ÙÒ¾éµ:à¿í™pŽR>¿ïî$ïßvPSRpsr3FGL J2035.0+3634PSR J2034+3632?ˆ'Q¿\-?Œ½gݤÞ?í1{<Ѷâ?·Œ~%3µ?³o;ᆹ?¶ýÌf}?z:ï¨åÀ?ˆgØ,~Xc?ëАKRâ?»Ѷ¶¨?¿Û£^ªÚ?º«·ÎÞï?§µw'BÝ.?–bÃ7"vã?ëÕû÷?¥Ö«•§>+?¼/¸®±²?¡¿ñº¼?E«óðŠÍ?7ã±Ñž—?ïáH~l?Œsóλ'?œÖwP¸8?ŒʤÃ14FGL J2039.4-3616?ïóûuŠNVÀBEò×sÀ:`
ôGÀ<œ£äv6¾@­ùÄ|œ3@Ží¥,u?ÀX[
è'N?Ù©íœ@(R. ý@–ÖÇL…?À×½ìŠ,¿ãˆÄvW˿ڟ[O7¿èŸ5_ˆPÇ¿ïþ£ßm¹A¿ï§匷3PSRPSR3FGL J2038.8-3613PSR J2039-3616?ê"6Ñ\¡Ê?»Ä'%áQ?¼	ÅF¢zÚ?µø|$'í?®¹\ðíÀ?§
'WOE…?åŽ `;%'?Åña@ã¬?ÂÄ)€fä?¾Í}2¼±?ÇTÿ×?º™ö²DS?áîC.'?µ­Yà[?Ò'eeáhJ?²´è`½v?Ç©|'"½%?¥×óƒç¶?çi -ã?«ÁŒ"¦!¹?Ätu"pÊÚ?©"ûôÓh?»Î®\û0?£œB½ÈÂ4FGL J2039.5-5617¿Ù9ªèî¸ÒÀB'ÁDŽPÀ8êÀ<Èe^ÿj@rŸÚ¦T?ÿ©D1ˆ8?©Ólà9Lc?ÎSíèÑ:E@#_'`4@6Öd¦à¿ØE2¤—ú]¿ÞÏ|_LØ¿Ýhã«5£¿âfB
f‹¿ííC/)¹7¿ïÿùëñPSRPSR3FGL J2039.6-5618PSR J2039-5617?Þjí¶È?ȺßÎï;?Ù°VÑÎw?ÉpYñHÁ
?Àj|'Jc?¶Ý'/¶çw?ÊÝì-«>?ÉãÖêºÅ?äTç˜k¶?ÏÕDª^I?ĝêup¥æ?¾Àº¸‡ˆ?×ê5¦G¼ó?´¾¬ÃlÕ?àI`"yD?µ‹'¤?¾%Cú?¡Ô?þÎK‡?ÑLî±³L?±ÄšsŸº+?Ü梖
?¶â¨f·?Ò×Ìn¸<ª?°ÏâvÒÉ&4FGL J2042.2+0245?қ¦ïÃqÚÀ7	üȽÀ9Ù©?ÿÊPÀ<QÙŽuy@ðªÏ÷Ð@x½ì_9K?¾­odfÜÙ?ä"_¾+Ÿ@@ »'-ºMn@¥P<³?ïÿÿ^ðP`¿×QN¼¦Žõ¿áš'ç°ë¿ìúE`²Ge¿ïþú¡Ç:'¿ê–­ÁnʹPSRPSR3FGL J2042.1+0247PSR J2042+0246?°cfêB=?¶‰9Ӆ?ìÎH¥"K?¸õ£(?÷?¢T±¡"PA?£3x¶÷Õé?ãD6¦M?šÜwµ÷š/?íO¦'9Ž?­*¿m¶v?¬ôÁÑ?¦˜ïlþø9?±0q"^ðf?›wۆå¨?èDzû9ü¾?­¥ÑÛIî?ÄHûPè"Ô?¦ößö¿1?y}²¬ûhx?aT»ô†¬K?î6="—z?¶Sv'…,?©lx87Q?œìØ,uVï4FGL J2043.3+1711?ãvòôþ­À.¢(D€cÀ8H…'òQÀ;½·ý1ïf@f­ZÁ—?ýÿ´€¥¬Í?¢sz ,›??Ó<ëƒFF
@0©:÷LÓ@Ú>›ò{?ïÿؒӬ»¿Ó³ÚøßzN¿Ù Ú@'ãI¿âŸ>HÀc¿ëò¬MÑD¿ïÿÿ)@k*PSRPSR3FGL J2043.2+1711PSR J2043+1711?±RèY'&Ý?·þ;õº8ý?ìoô…0*y?»Îi½ùá]?¦Zæú¯
Ë?¢]wf¢¶?™SjD`ï?¡ïn­'Õ\?í£†{RÐV?²šŽ•<L?©ã(ÏÊ8?«ðE+p÷E?˜ø·š
ï?ŽæxôΘ±?ëEù³Ð¬
?§ª¦ŸÝŽ?¿'zøî?¤c%¨Â£‹?T~vsG?MõòüŸÏ?í­É"€®É?œ¼¼§<†?²?»r"ä?œi¶¶›ÖD4FGL J2043.7+2741?°A©ìÃ¥@À"Jeà.©aÀ9sZôB\œÀ<%ê°¢¦@õ'¦¸'@+e˜U?¶'«hÎös?áëaŠ@ ö²(ܘ@ÆÞ	àÿ¿§˜»"Ujk¿Ðg°Ql¿ái¬}Ãû¿ì¬#ßÙ¿ïÔ÷©i^¿ïÕ@¿ð©PSRPSR3FGL J2043.8+2741PSR J2043+2740?À½¬ˆ[:?º^QØ×`?èð \ˆ¿?Á 5t}žë?·!ìeEö?± ëk"?®Û¾øqîC?¼a£—Œ=Ÿ?çd¬Þ‰?Ë0"}VÔ¼?ÌC€0
M?ÆD<œœ3?ΑæÓb©Ÿ?±§çtZßã?åeœ
àžÜ?²	•?‰w?·¯Qê5µÜ?šæH­V…?º}ŽÜ?œF+$?èÀCù.zO?±Æñ'ƍ?¿ùcý¬?­p"âff4FGL J2045.9-6835?éÇðôRÀA»>ÄaÀ:âØK%À<ö¥Nفç@ßé"ÃÏM?ü<cþ­©?Ë×î©ksÁ?èô¨H‰Î@uh¿ÜúA@"…£Ãi!?­t²ÄL¿àÞç+ž¿Àøÿ%:¿ãz›#¿îR£`—ÅY¿ïêÈ@ +šPSRpsr3FGL J2045.6-6838PSR J2045-68?¸ùÆ]
­?ÀùCœ—D|?ë.Zôëæ?Âl¨ž
?«&Ä‹çx?§ªÑª•)?Dz4¶p?À'߆«?åtşó?Ƥ>…þ'%?Ã)þ´ÉÁn?·Š
/'^?Å"ÿfQ<?¨mŒD›¾?欹⥞7?°&/hx?ÀJõv5è?¢:†^¨v?Ô#Él=Ï?³Œ'[;·?à>¥ü­?¶ãsØ?ÆÀK]4Ð9?ª–ç·¢
ô4FGL J2047.3+1051?ì¹"Æ,0À3º­æW¸NÀ:K¼£n/À<8öí1Ç"@Tö.šó?û4+'»?Á†}]"ñ?ØθêÑÆ@£'üÇf[@¹ù$¹	¿îü¶¿š4I?½_e@KŸ'¿ÖEìuæ¿Û
b¿ù¿ëLóc9‹<¿å€Þý{ì5PSRPSR3FGL J2047.1+1054PSR J2047+1053?ꙭ`{¢Ÿ?¶ ã†?³O?´‰¡³*µ?®×¤ÓW¶H?¶¨óÜoÀb?«3Žá¿Œî?î¡&ÄhWn?£TÆl¸?wöÿoÆ"H?†ÝÂÄõµ?¢î³ËÄë? nϼí¸?ávÒ;8Sš?¶N{ã}LÌ?Ñ-|'ûS?³ÂZÒõ˜?Çɽí("ó?¦ÜowŠÓ?êÝ8°úû? šä¿
ö?˜êy@î?'BŠ2àò3?ÁmÎùÓV?ŸÕOeLòë4FGL J2051.0-0826?­½Š™À>cC,¥zÀ:š~dž;ïÀ<¿,Áÿê1@›™¡ýj@o	A=?Ä©h?ä¬(²¦°Ù@Ñ'o°'?ü÷WØYý¿ïÿøþÙå9?ïÿ¼]éÀ#¿ÊöˆÝߙ®¿áaÝøï¿ïÿÏ"èbU?ïõw`‰­"PSRPSR3FGL J2051.3-0828PSR J2051-0827?ÊVfæïˆf?ÀtZ¢"[;?èɊ‹äÆ ?Áƒñ¦Çp?"wKêøã?"L½0è҃?¾yӔùÕÓ?¾Mö¶>¥?èA>ma.Ý?Ç,£w"»?¿|8ÿü³??ºfm ?ÀËS™Î?§ü«¡÷^?æ«qÈÁúp?°â'0Ÿ)?ÁÒ!¤|p?¢ñŽÓ|o?̦*‰Ì^Ø?³þڊýKØ?åuÆV=Ý¥?¹œG…;]?»x:xU)?¦‹ãÑT4FGL J2052.7+1218¿ë·ÄaÀ3ýµc#»ÇÀ9äÂa8ÿüÀ<(2áԛÎ@>"«n@8Ÿƒ¾f?½–^%Ð;?ÃB'_ŽZ÷@ûšþôg@à?¸o?ﱿàÖ'¿án'xbè-¿âÝ6;ü/'¿æÓ\.§¿è0dxO¿ïíh]â^YPSRPSR3FGL J2052.7+1217PSR J2052+1218?ì-ƒ=¬z¦?° ñ¡æø~?‡L¹Egp€?}€C
|\‹?»ªNéï<¼?¯NvQ?ìk¹òŒ?²ÑøV¦Ä¨?›k]{…¹ß?œh¾¸lF'?µÌ2ъ1?®ƒÖqŤ?ëEQI÷ý?£ÓêÿLzd?›ÓyLô‡Ð?‡[ÛtÙP?¾à•2s!? ùôÁU¤?æÄ
¼?¢®ü)'°?¹°ÿ@(€?—G5!2?Ê·AncÀÑ? sù kå¨4FGL J2055.8+2540¿‡ÐöDm×ÅÀ)
7.jwÀ7ªÃvõØÀ;¨ÿ°NçÅ@KüŽ0"Ø?ýpä8ú'?ž:öËù¾?âËt8Ùe@Al?Ä;.@ñœs)˜?ߓ~AÏXB¿«,F¯çº¿ÜÉ¥%	ó¿ê "àwN–¿ï z"Ԙ¿ïÿ atd+PSRPSR3FGL J2055.8+2539PSR J2055+2539?MüW†DÞ?K=Ò$Í*¤?ïÑ'iʏ?v "Œ2?s¿3ÚZn·?sžóǼ©?wÙ"LRŠŸ?‰½Ûk$}W?ïÖ°w—š?­\xòwy?˜îá]øjF?«†lœÉð?'EDiÃP?'¼ÖLwªB?ìÒÙ)Ýöm?›‹;]•È~?´×ðõÛº?˜7ã3ôl>`Ôk=9pQ>r"WArð›?ïé]"~?f>S:N¾½?f¢R%B«?f>I‹‰'™4FGL J2111.4+4606?îÛÊõé¿÷Dº)\ÜÀ7Ä 
a'ÒÀ;Zƒ®Ò@iÚקqI@#.£yè?ž¨e—çñI?а.[ˆ@,Q¾ôœõo@qÁcb%?ïÿ–¹‰$¿Í}÷<7ç¿àø¦Ú'Q¿ã@5z5PD¿ì¹Fk¿î<@".þñPSRPSR3FGL J2111.4+4605PSR J2111+4606?"÷¦JjŽ±?•Ñ*ÊìÚf?ëÃêÒ$7	?»"ð.ÐÓ?¼â¿ÜC¤?·ÿ«t\f?…'6}?‹öÒÁÚÚ½?ê>_§l®–?Äb	^e Ý?Å´¸Nå4'?Ãô',õܗ?¨§½²'¡?Ð† Ï?é+ëT
­?±"éH™u²?Å&h§6?ªKÒwÒT?@Æý5
*€?5¸"d'Ý?îŽ`újíy?Ñî̇?¦ÖÔd|ÿÕ?¶ÄI¤j4FGL J2115.1+5449?æfùѽ¢b@{>—ÔÀ9«Ã½Y'CÀ<H:vôS$@ AjT‡–¸@S%A(Ï?ÀÞjÄoF?éyvCS;ç@ Yªu[Í@5euû…¿ä'pÀ²b=¿ßò([¾Âž¿j‹éÐ
;e¿Ü=eü‰(¿ìòª¬çT8¿ïÿÖ"î9PSRPSR3FGL J2114.9+5448PSR J2115+5448?Jw|¿O8ˆ?NÆù	¥@û?ïµ"¹óOˆ?ÁœÛÕÂ?Ù·7*_?ŒÓq‹iÛA?#óÁÿ#ø?'®Çg0ã?êeNÎ1£¤?Çb]÷÷£?ÅX…‹/?Æ\k°Z?©
%4Y"?–¡3H£Œ?êS°27?¨¦g8·Ÿ?Àmõê›
,?£5܏­¾ò?bìïÒp¯?Vš\ðh(c?îã"(m3]?œ4©©2? ˜ôš/£ ?›i݀¹4FGL J2124.7-3358¿±•2BI0ÀF¸øa¦
EÀ7ú=ú	FÀ;Óc7ݼß@꓇0á?ùp0dKÙó?¡¥€­oÊ?àÿ‰kV@=÷Ú+Z!@)‹ê"n?ì0`†R•?Ĭ	É,"B¿ÐÆÚ¯ä^º¿ä>÷âz3"¿ï"NB_Ì¿ä±ÈcäPSRPSR3FGL J2124.7-3358PSR J2124-3358?pK%Eàé?ŸŠò?ì0ؙ¿;@?Æùú…cì5?º](h´­Ä?Ä8‡¢š©?Žš²ÏîEþ? Ñ]C@/?îƾe¦?·ü*‰·>?§-à0?´°L⁲A?œ
rdè}D?§æÑÎ/?ëbäÒ&?§""7Š¬?½ì@4¯û?¥u~ùF>¥!ì	n:>°Ål"èœÐ?ïºÙ+€å«?y2Ó£¨	.?I`˜o?y2Y¼Á4FGL J2129.8-0428?Î*¯ùNØMÀBz弇Û+À9»†ýX†À<WêpKÂ@PV¤&c?üûtëdg‰?¸+ƒ–%F?ÝN-?SR
@ 4)ˆ;£@)nÑnòý?ïøï]€¿²ê†qÏt¿×Â??°ï÷¿å•yyh¢¿ë·ù1~'¿ðPSRPSR3FGL J2129.6-0427PSR J2129-0429?¬N—Km÷Û?¥¤rƒ?´œ?ìŸ÷€=¦?´ß"'ÇÃù?±´žGî?ªØx:ȦØ?«ÛÓ%"°?¦)Mfñ¿?ë=uöQJ?¸óÂÖU?¸)²½ƒ4×?²kŠ«Ht?¡fÔ(Iý*?zZ¡(#z?ëgò·Qß?¤ÖÇr&b?¼ÿÖ rx?¢!ñÐÎò?¾<)Áރ?  [çÑQ¨?äñٜýîè?²Í…Ιa'?Í(ûw'U?­ZýXŪ4FGL J2140.0+4716¿¢‹y~ÉPÀÌ~É3»À8X«m×sðÀ;ÈY±L=Æ@3xÁ1ãþ@}`ݐi?¨Gq¿Ç?ä¹V}»Â@2fz–¼?ûÃrƒU4¿ÐË+!–Ó—¿À¯HW‡¦R¿à}·³àm¿ëSž­ÕÁ¿ïÿr;†¾Ì¿ïÿ÷Âé±PSRPSR3FGL J2140.0+4715PSR J2139+4716?hÌ´Ä	^!?pëZ VÖÍ?ïO°'†½?¡M®z˜?'ðY7-ü¨?Ÿ1³
Ãh\?€+î°&ÂI?˜‡-æőW?ìG=‰8èÏ?½™O—T´v?»À•à3á>?ºÇ'¶m¡4?"ªf:?'k3û_öl?ì§DS‹òº?›ÅYœ©‹s?µÛ9ƒYД?˜'ñ*œ>Ù
~¡=Î>Ó½?ܯ
?ïÎՀkv?nA̤?xŽü¥H×?nœG˜À(4FGL J2205.5+6016¿ïö]?îz@
è<v©À:zD& }¹À;¼š*¹@"5ÜP£@¾mþ
?Þ
üÂÞ·[?ïýÖZHŒ@¹'m-*@äBtä¿ïÿÞ°ô)?ïÿó5bB¿ÞEÿÉú5¿â…¾'bE¿éû/¶¦ñ¿ëù¦_$ӟPSRPSRPSR J2205+6012?½—õî¹î?·ÛËôR˜w?À™û%!_m?¼³ïN?è&'xàjd?Ãuý`/"¿?¿©†X²ÞÛ?¿‹îrv?"?Ô`ŠÂ¤µà?Í̉þ·wl?áډӗI6?ÎZ+ûb'/?Û!-!U·y?®p¼Ÿ'î?Ã3¦Ÿ¯?¢õÒ²Uë?ÛED‹Zpþ?«'ØnÑT?Á]R·™—?©ÿÏʦ ?Ӎbcÿ\³?À1°"?áâùRk@?À¢³/J4FGL J2208.1+4058¿­øí‹51À(/ëkôDáÀ:ÚøßzNÀ;÷։1@éÏç3€`@=r6~AN?Í&¢+8'ï?èÜsÔ
2î@
ç-@™Á1¹?èQpjÌ&µ¿ØTfB
g¿ì|º–¿åù`ß=虿8ˆÊ¿ïÿ5À+SÁPSRPSRPSR J2208+4056?âÛX­ÉE¾?Él°Æèi?Ó
'Ÿƒ??ÆÿLÖ,'Z?¼îös7Å?·²G7¸'?Ñ ;y"ÐÎ?ÊIñyã_ú?Þ]'̚Æn?Ð!SX«D?Ђœ¹ÑhÃ?Æ+‰P>§?à™`ª2è?²9€.¼?ÅêJeâì=?¦9Ÿ™<Ú?ÓØ'º$?­\×_Ð_Ê?¼–AÌÐ5…?ª¼ïŽ'º?è"z'M'2?¶«ë•_?Á*ö|a v?¬)ŽKŽ†4FGL J2214.6+3000?ܨ&güF@À5¬9-Œ*À8)"UUÀ;Þ\Nµo¹@û—OgqS?úð.½§?£U$'ìG?ßmrÿÑÜ×@9ÔfõŸ@§]žk»?Ó˜ÂÚÄ¿»ã3–…h	¿Ö\²3¿äʵ€í ¿ïÿéYËMq¿ðPSRPSR3FGL J2214.6+3000PSR J2214+3000?£ÑD–Ó?‡âÓ ˜"€?ï–ø͗ե?'rüÿ?tàŒbЕù?~ÔÐÉ?LüÕEm÷?¡¡ëU^Ê?pî|Œ?®5
<aË?ŸÄsw·_?¤‡.—­k?"í^À?…	ö|Ã?ìí¬›Ý§ò?šå,bˆ²8?³—ZÛ»I?—©'~Q–<>ò‡ârŸ>üöÃa‡ž?ïnDG·]?…)2ÉZiú?'2ϧÁS?…%¶¶à"Z4FGL J2215.6+5135?éN·¥-OÀ­6 ¥ýUÀ8̎eˆðÕÀ;þršQO~@kÛÎóB­@—‡B_ ?¦}	bvº?ÒÅ-¼PÓ­@#%">5ŵ@Wå¢0Áê¿·,£Þ'N_¿Ö§]CýÜ¿Ü-l…]¿ãý/5w±¿ìg ÉN=¿ëò¥Z'"PSRPSR3FGL J2215.6+5134PSR J2215+5135?oÛg¯
š?wæ*½Ä]c?íÎÛyð¾I?«­|¿¸\?¯$Lóþ:?©ˆ:ØÌD?¦¬œ²Wa|?³Ü´Àê•Î?äÒD¬¾dó?˳Cýä?Ӆã8Iê?ÉHžéæL¿?¥‹m#EJr?™Tðj?ë{5&&s&?¤¡Ó5=Èï?¹` =)Á¢?œÌ\ò\Ýÿ?§20"D"?/5B¹¾)?êƛV8Ó?§Uwì9†?¾2²Ì—)?¤yIî"t4FGL J2229.0+6114?ïÉÊl}à@–Ü»WYƒÀ6þ"ÅõÀ:}E$Í>ã@ë
ò[ý'@h
"'r5?‰¥§Cü.9?ËçÂÇeYÌ@A[5Ÿôým?ÿ2̾_ Í¿¢T(÷(¿Øj¾[›¿âÓÄ"ïï¿åXåó€¿ì;E»Ëó‰¿îá['—PSRPSR3FGL J2229.0+6114PSR J2229+6114?qç_ßG?s8Vލæ0?éúšä´ ?ÅN@ó´?džYn5ä?ÄÞZ1» Ó?hÝåï zâ?‰VNþ¤?îÍ?Ê7}?®g}$?¡ž0Dj€Œ?­©kñ?±u'é¿?ž¯&@ŠN?âÝq–§¸V?µ´K'c'?Õçµqö'?³ãq^"Hþ>UÈ|·šM‡>p-GËãe?ïħѪ?|÷µê]XŸ?}¬x‡wý{?|÷±Ú1ßò4FGL J2234.7+0943?ä§sMlÀD8ªà"À9WÿÚ@SÀ<*øÞ£@ 2×àÔ@-»à~í?²üPý+?Ú=ë]†˜á@!@åæyF=@
£Àäâ?ÛÛ°•^¡v?'9jYåúp¿ÚîädC '¿ãf0€ÑK¸¿ëùd€LP¿ïÿò^VÍlPSRPSR3FGL J2234.8+0945PSR J2234+0944?ÂO3¿>²+?¶ÊM?¿Ä•?ë¶1–ç?·¤×ÊÒ#?†_7Êo#"?…$ã
ùÝÈ?ÅȕºßO?Ä:½•Ó@?åÀ䪤"w?É"âc2`?Ã3כgÒ?»c¼CÑ͇?ø'c†C"?±®N%Š?è›ö2`ás?²
•ÀéŒ?³¯I¥ìn*?—I_fRò?̀	µnù¤?¬`Tž3†?ãõÛE1?³œkkåôÚ?Ç(Ý|B@?«Îêü³«+4FGL J2238.5+5903?ï0.úqÿ?Þm:åÚÀ7tKAFò-À:×¥œàv@ßùߪu	@øB0üø? mXaÚªJ?Ó£{X)b@1¶®::Žq@=ØïÅË&¿ÈçV¦Tèæ¿ÕZºá'׉¿âø¾eUð¿ç‹Ýž¬(¿íÏ@ãȒ¿ïÿ÷œ"/¥PSRPSR3FGL J2238.4+5903PSR J2238+5903?b#€fÁQ?aàÑD¥Š\?ïb.Pj0?'½¡ËoýŒ?'yьeáÚ?l:•¦0?tPj¾Ä¥Õ?€(®¦ø©?ë\wQ?¹lK¯<Ž ?Áí0œ,–Â?¹@÷öºu?…xç<Ý?tý'Båæ?ìþ¥oþÂ?™\'lä$ñ?µ` ·˜†O?–ï
;´?µÐ†XØÇ?ì'2}E\?î ۈ`Ú?›àvÅj—?­êš\?›Ýað4FGL J2240.6+5833?ïiBuÄ¿¹äÖg3À9eNÀWs"À;'ÊÇ9@¢	ç4'@Yr|õ%?¼*Ë/¾´†?ԞG=×&@³q*Ç?ó÷Œo?Ñ6þï´®?ë·3ÞSÝοÝá'ÑÖ÷É¿åÀʀAXæ¿ì䥜[d¿ïÿ¼ä!}(PSRPSR3FGL J2240.9+5831PSR J2240+5832?ž+_õ:i?'*ð}¬ä?ꙇÈÑ@c?¹ånG`:·?ÁÔtÞ±R?·ÓÜ,	%.?‹|‡ÉäÛê?CSêÆ?àﷻöà?Ìú­
f^=?ÝD¬J)kb?ÌÝGÛŶ?³€£b64o?˜rw¹JØò?à»ÝâAŸ
?·ù¤¬Ú-?Ù¨bï4Ï?µvBê,Â?Š`ØÜ4ã?r½vÝjZ?ëâ	`)?©;¤ B)?Â>jN/7[?§éê¨ÿÂ4FGL J2241.7-5236¿ÑP‰ÀKw' ÿT	À8e½²}–.À;…ê&yçM@'´§«€@Ôœ¸2?¥W]bW?à¥Ç¥EŸG@6üa'?þr܎`ÖZ¿°±×þÚ,?£PAá̹,¿ØĤà¹)¿äƒÇ4ÝW_¿ïnàR»Ž·¿ïÿ»ËǔPSRPSR3FGL J2241.6-5237PSR J2241-5236?]Œ)õú+¦?s\­w"Ï\?ï¬fØu§"?™Ú.B]_?4Ä£ÖÕi?"í©ëJn?Ò¼HãíR?›ÍßŨÜ/?íÒTK8l…?´ÒœŒE®K?ªq](@ô?²½ŸQo~C?†½0­o>ß?wÚ'ê
u?íTuŸ&)r?•wµ9º?²"¬ñ ̋?"oµ!¦k>Ò!7| 7>ÔÍ7}Þ?ï)'ŠWÄÒ?'IæLåøY?šÎŒ¡›Ï?'I§ŽâAú4FGL J2256.8-1024¿ìlÉlù†ÀM#b¶®}VÀ9¥[n¼À<EÉGÝ@Ž%·õz@?ÿbîᵒ?µ¿'Ò€?ÔGÁSœà@éö©?)@k • ãû¿ÒEI€|'"¿Ó¶z¢Þg¿à*‰
ÖØ¿åEcKÿ²Ó¿ïÿ/àîAè¿ëw´!ZBÂPSRPSR3FGL J2256.7-1022PSR J2256-1024?ÖЮ‡"åR?Ãà~1?â	+0$fü?ÄñßL½¸°?´sì`‰2×?«añ0?Ö~12jì?Î3HážÐï?Þߊ@$‰?Ð'C®q?ÅD‰áø½?¿ü ¨S¼A?Çó®5O¾¦?®î'êû^?åÙ
ŸÈv?±'8??À¨KŽi?¤vxK0É3?ãyûLnƒh?±CrC6Ë?Åj÷dæu®?«ÞrV´?Ì­i_|³?©¦×£µÚ¼4FGL J2302.7+4443¿îÌÅNkTÀ+ü"«%³À7ý#!m8À;ŸDÔE@§ó3üÝ?úæé¸?Ÿ7‰.<~a?ڔšCã…@9AÅ3?öŠ¸³:T?ÒCÛí㿦ašNË?.¿Ó$"ô÷ŽA¿áÓ{½™Á¿íFñVI¿ïÿ°"—©ÕPSRPSR3FGL J2302.7+4443PSR J2302+4442?iˆZ™J
?n([ú'RÎ?ï}d0/9À?–·)žy?ŠDÝMß
l?'÷¹é#{?ƒ°OJ¤}Q?KyAÎ(?î«¡¯,?ª—	æm? cÂd÷?§_ݾò'Ì?oƒ_îâ?mŒôÉTì?ì²j6â7õ?¢8¤Jê€?¶~½ÝÂ~?¡yw¹…s>Ä:fr€>ÌÍr¦šC?ï…ô–݁?'æ3ljáï?Ž–¨EøÐ?'åÔF¦D4FGL J2310.0-0555?êËß@åíÀLó5*"8	À9ñº
RiYÀ<ƒ6ª¶øO@bsN×(›?û_틉5ž?¾rø-}½?ãáKŒ]@!#{ñèæ@›ûcŽß?ïöý»'"?ÒýŽ`«fv¿ÓfF…öN¦¿ç<ù jn3¿í×ÆZÂÄ5¿ïÿøÞ£ŽæPSRPSR3FGL J2310.1-0557PSR J2310-0555?²\e€±×?°*[K?ìÑÀ™WDÓ?´cXv7p«?œVVÏž(?˜ÊaŠ^(?´‹a'OÝ~?½ŸqHŒ?ê±ÓÔ(>?ÁØ{DN?µæ?àš?³g[œ›/i?±#m;'^? |ùê´zè?êŒøfÝ´(?¦ËuÐ׆\?ºtύ€L_?TÁs?Èt³,=?­—ªºv€(?äB¯1}y-?¸'ªªjc?ÆíΜVï?­ÏÍó$4FGL J2317.3+1433¿ï½È'Ã{ÀE;^Ès¬À;•'àÙìÀ=$)Ùî@¾CdÞØ@'#[NÛ/?؈•zѐ?ïÿ–ل@£ÃÙß@4ÛÐË´õ¿ïÑ	ro‰%?ïüٍ©Ì¿ÔóÉ[(Dÿì¾YÂi¢¿Ð×ͱÏ…¿ïÿM½øôsPSRPSRPSR J2317+1439?茲©Zã4?ÄÝ×7¢Ï?ÆŒi
?ÁŸc}ö©'?®º£Åጡ?²Ao!¸ç¿?äOÓçÏJv?·ˆoñŠ¶?ÇNpÁ´¢r?É̹"4?Çr?Ÿ3¸?¿¡Íî·?å'ÿ`>-?±Ï‡ØÂd?Æh¥z!¶i?®õšmo?Å]ˆ]Pá?£v†hd¾þ?âg‡d—?À¢8rVŒ?КçV5?ÁºôƒF‡«?Å,Á7¢?¸®-÷#GÖ4FGL J2339.6-0533?î<âmŒº'ÀO<Øý\·'À8Bj4Q@À;Ítj5(@à,Ä.B´?úê°¢¥²?£ÓցVÂ?ҝ)[™ñ@0í·'êy@é\‹{õ?ëVáŽ$ñ¿ÒÅ}Î¿Ö.ºJi¿á^n€[˜¿ìÂåÃ=Ø¿íˆdüPSRPSR3FGL J2339.6-0533PSR J2339-0533?§uwˆÕ?¦ß'õp›Ë?ì'ڛs ?½7[ÆÒuh?³¤g'?µ(LDØ,[?¯¤;–q?» Ê¼"?ë§Ô7êë…?ÅXÎݹ?³8"ݕ?·ò÷ÞVèT?£2Gèff?˜ ÿÏÿ?ë;-©`çý?©>äÖÉb?¼ŠŒì?¢ç/œ_J?pŸöoª¥ˆ?hþmÝ"=?ë:Ñb3´O?±X™×0ã‡?ºÃ³Ù›?±äèD¡e4FGL J0002.1+6721c?؎*±b@Â[T‹À9Ð'Ai
À;2ɪ@o£c@ëˆÊ>}?Ê©>þž?ÖmŽcZ˜R@¦÷ µí@S³Ü:ÿ?Ø3ºâ¿}Y¿æ­ݨ<J¿âžâ^.‰€¿éB"ßοïÿþ½à ¿?é§fN³OTHERunk1RXS J000209.4+672503)?ƯÁ*kì#?¸=æWS©v?Ï÷‡Ùµ??¬öú-Á?âVH"n—¨?Ä,Ÿðs?Ï:#Žæ_'?Ț°*?ʲÝo«?ƆY²O˜Á?ᄿ×ꀱ?ÉÐyÅKî?É
-·ÁÙ?¥'Oa™'x?É°%ÅÓÓË?¨)KVN?ãQk šÅX?®C–ç?½ê¬ýkO?¡ÌcÁ»ÿ?ÀÝl»?¤Ñ
‰{kO?è<sWãÑ?¬B@/à`¥4FGL J0002.7+7220?ï‡sRnH@#¨–»˜ÇãÀ:hã1" À;}¹?QN§@e	Àóû@H_ÐJ/Ï?Ð<ÌÄ¿78?²[¿ïCÅ'?çFùž¼ï	@HF6p)‰?î–ÿöÅě¿ÖOæ<Štä¿å	Ñ:×B¿ä"è™¿ï'Æ0ÑY$?âãA&
OTHERsppSNR G119.5+10.2?á!Û)¦K?Çø(O³"m?/–«rM0?€ÿuôl,?Ý3g"Q!?ÇúüÌô?å@NøVö+?Ì¡€…i}Á?'Ï›«? ƒu|Þj†?Ôbp¯Xú?Ë&ˆ²þ?ãM"‰¢?²E9÷›]?§¬âáèâ?'ú[œ×À?Öo:¬_ŠÀ?°•+ëQkZ?äý]W÷7¢?²MsÂñ?N€/kƒ?"<=ÃÉ
?ÕBÜ_?²
›ƒ‰4FGL J0024.0-7204¿Ù€°á×ÀFr¾ß¤@À8Yø©ÊiÀ;òkón!F@y§¯†ì?ûäû,[¨?£g¿j?Öìþ{E›–@4¸Œ£è?ú"Ï»¼Ë?ހeëí#"¿¯kR3~‡š¿Úàr%uZ¿ä.b"óè¿íè«ð´2¢¿ë©;}"OTHERglc3FGL J0023.9-7203NGC 104?mNSº×W?pBYbþÌU?îîç©`¦j?¤<D•R?žyGis×÷?¢™'æоo?‡>#'+¡'?·C hñ>?îás²zV.?£ôòvArÉ?˜2wèi‰?ÒŸu{a5?	›ÜçBÊ?€óa¤[P?í®)]°'?žƒÜH0ú¥?³à'½Ø«=?›v>Ö>?"·Ù`ȟ?#M$Ñ;3î?î÷A6¤?'{ŒMÆê? yèöS4ÿ?'kô&¢—š4FGL J0025.3+6408?è4ˆ;"k?ö¿ã°> ÍÀ9Yº !ÞwÀ;'µ‹g§¯@ "CÆS`û@dŠ=Ü¡?³á_èE?ˆ´¼¾?sç?ÖH¿aÕ2?÷>ó/âò?ïÿjCj¸Û¿Ê˜†t"è¿Ü•qaEg¿åÏ2ؚ`i¿á"?Žò¿çàÌÞë]\OTHERsnr3FGL J0025.7+6404Tycho?àÌމYü?ÃϏࣇ¤?zÐZ'r9?wëZ®ÜO?ÝûƒÓƒ#?ÃÊXÇكË?ÐDG3é¦!?Étžþ!<?›èĹHQ?¨¼˜"Õ?æþ–@@ëý?Éç<ÎÃ?ÞHV¦'?²7Éþéç?©'ГWý?1FE§Lò?ޔøÿ['?°»ˆð"?ڱ߲¤y?¯œäy)l?Á¾ç³ÈÏ?§.È"'´?Ün¬sw"?°=Uœe4FGL J0043.2+4114¿ÔõeêÕÌÀ5š¬§"W`À;
"ßþعÀ<fI¿f²½@-¤€¨[ÿ@0\"U?Õ'،°?æPràÈ,@M7 '½´?öؖVîú¿ÞDD}ˆkõ¿¬¸€‡qú¿×Ç
â@Ò¿îž/á5¿ïÿ¼þùoÃ?≲€ñ,(OTHERgal3FGL J0042.5+4117M 31?꧉|w³?À';ôæá?Ÿ‡®—6ð?¯è=À
t?Ápö˜PæW?½.ýýʔÔ?ä.›7Óʤ?Ñaºê…?Îñyïï‹+?ÏE/µ¡[Ò?ÀT0ÁJF?¹9ƒÁ0Ô?à—½í×6?³zYz&?ÐÃìÔ—?±¥G<\ ?Ío"
 ù?«ñ€{êՃ?×£Ì^‰ÀX?²ê¹J®ô?Ç2*É*Ç-?°'@£Å"?ÜÃ<àÜ?´"Ž·fÐÌ4FGL J0047.3+6943¿ïõûÃ
@iìb"IÏÀ:ç¬è*÷%À<TBcQÞð@!BcMØ%?ÿ*'5Îîæ?Ê=£N¤(?¤0bp-?Þь"Þ ²?üë¯Ï;¿ïÿª¥Z—ü?ïø;`(^Ä¿åÑ3~²†¿Û"½'Æf¿Øþìɹ¿ãMòfºI=OTHERunk1RXS J004724.5+694222?ëïÀV˜©?·)¿¨µµ?Y•¨<عH?TÎ
δ?Àm®+ëì?·
ÏUÔD?á@²Ñ¬É?ÊY¡"n¼]?VbŠ—ÌÅ?"øñXUÒê?Ý@ÒÖG=?Ê5
"¢Ë?é؅DJ,i?¤"Ï$tn?ˆ‡˃®:?s9þhô8?Çy²z?£œ£˜Ù,'?鱌´¥ ?¤hþMOÛÌ?eqŠœ?E°"…¿?ÇCvPÕû?¥xo¿S;ì4FGL J0047.5-2517¿ït.VÁ•ÀUþ	þ†ƒ<À9¸×ï?¾\À<'~b¯@¿jë@,^,Ü?²zãáfaß?».Ï¡=|ã@	þÂé<@RÙâ)U?í8ÙÀ¦"ê¿Í]ª?¯…¿áÁVw¿ãú¯É†Ç/¿æ´EL:k6¿áágßjrOTHERsbg3FGL J0047.5-2516NGC 253?ìÑD"œ½?®Û½6¯?|wþ °É­?u;l: Oa?·®_¬à
r?­'Z`ó®‹?îëù«U9é?­µv!ž˜ý?¡tp¬?–pû­ó¸‡?™÷ùÛ ¸½?§œuñ	?ë¡Â"-µÖ?¥Á¤/kB?¡yy;‡?'F9ð;?º+.ÔÕ³–? ÖQóv=?ì·"YŸ‹?šùš`5¼?ŒsG¹=??zÎQ=&Bí?¶¹5ûÜ?™>¦`‰oR4FGL J0058.0-7245e?éNÐà$9èÀF/Ne¾ ºÀ8f֕£jÔÀ;~ÚÉÒ+@<›=އà@üÅ2¤—ú?¥ª	ÜÖ7ã?·e~"é×@ò–pm@Pބ°(|?ïZ˜1º/¿Ü°žBö ¿ã1Í7U×£¿ãdâ¢÷ç-¿æí¾Ña‡¿ïÿDN
ª
OTHERGAL3FGL J0059.0-7242eSMC?åÕóî¸?Á#qZIƒa?£¶@ýî?›žƒÈRÿã?Ñßñ®Ó?À›%ð³_ƒ?á¥Ig}/õ?р™êø?Ó6ø6Z
?Ð'@iÈ?Âüéõ،?¹JãÂ_|÷?â6š9Y¹j?±£¹,úá?Á¸"	ý8±?¦ê"ùà¾?Ò¶'MðÕ?®°Šâ²ù¿?áϏf`
ì?±4ÍÅÔ·z?Ç)~"ã%ï?°.þÕº¦?ÐÌ!èÎW1?°Ÿ"Šºª²4FGL J0059.7-7210?ìäHRîÔ"ÀFwè¢ìÀ;$¡¯ À<pƒåÓ.@;uÒêóÿ@¯0¿»lR?Õ~aDh¶?ëc݊Š2@4	t@¼•Dj¿îÍ=ø:?åüO{пç£ôÑΔM¿íç	Ÿ&¿ïüÖë3À!?ã'‰|$TOTHERsfrNGC 346?ìLE"~Yè?´åS†ÒfØ?°ÐÉÙf×ä?®Å¥ XÏ?©šL±¬?§É¼ØfFî?æ=?hmJŽ?˘<Ý]~ð?žøÑ[!s?ÆâLöÍÑ?ÁL	Œï´U?¶+
éËÆ0?å…í0æ?³X46»'¼?Ä­åÑþZo?­N`öu~Ø?Å:ejiav?¦æm¯î Ý?ãÆà	_ñC?´¢º.ÿW?Ê̌
D/?²æÕîf_8?Æd³NröÃ?¯tYƵ‡Š4FGL J0102.9-7051?ïýb¸ ´°ÀG¡ô±îÀ;@X|™À<Ȟƒ
f@ñà¬Óˆ(?ú¹_ÒÎn?ÙjCä'?éäNÿA"@uPÊï$@š6ù¼D?îð0Ä#¿íÝ.yÖ?Õç[ƒßH%¿æÐt!:k¿êÿsFT¿ï5?†'ÍOTHERglcNGC 362?ïX"¶ç6¬?šéº=
#?p Yà¦?tÅB>Ææ"?èÁ¡ø?˜Yx×D?î'Áúrý?¨¾d;9}?}Ûkü<õ+?ØÒ|
Ã?¤r×q1‡?£ÿñ?ìkÈŸÞ€? k?×Y­K?¢a­ÉÅ?"dkÖØÖÆ?³pè&l?š¿­ º¥?íšp&x‡?š(ãÕì?Çۜh*"?yu쮉yþ?°öq?6m?˜`k'íxë4FGL J0138.6+6821¿©Ënš2µ@ƒÅ¢6 MÀ9Á%q©ˆÀ;‡tߥíe@7fÛ¬8®@ú}ªOÊC?¿æùß)›°?³u67õdÆ?ó®K½m´9?íý°ðMZ?ïý'w>$ÿ¿ãþyC¿ë-Z˜¿çM	h^Ž+¿ä©,I4&x¿å¹^Æ^ô'OTHERunk87GB 013451.9+680621?äÑåá珮?Æýqôíñ?•¿Ñ±¨Þ‹?'€|ƒ¾ìò?Õ7!R¼?Æ»kÙe$?ÊQ}ASØÎ?Á¶ò‹é.?¾@fäÂG?½œ3L?壓ìîq"?†›Ž]?ßOe+žÖ?²úz]%?­€ù°–Ü?•ØŽ#À?Ý{žO;?²M(âN`?É®L6†$?¢šDœ-?ËÑ0i¦Þ?­˜üÌÞ¯ä?â  áHØþ?®Äò±(!e4FGL J0212.1+5321¿ï"ØÐnËmÀ…‰ïØjÀ8ÚÓC"LÀ<|ûÔ!U@Å0L£òŽ?ýàBæ.¢?«ØB÷¡aº?ؚÐÑ>K•@)0"»?ö­—}_§¿ÙÎ"Ë+b¿µèüoq¿Ü¨b_EµÂ¿åj	=ìIÀ¿îeÖS^Kæ¿ïõŠ@`B`OTHERbin3FGL J0212.1+53201SXPS J021210.6+532136?D3Sb[Á?€©–Ä…d|?é¸_–%ð?Å,®è…?È
>reBƒ?č(.±È¦?ƒE´¢Ã…G?'ÉmÁKÿø?ìA^ªg•)?½ˆ¢:‹"?»ŒTjæ?½an1q
?2D«Ëi[?zt›u¹–9?ì¸ôè
n? 4ò?¶3W-ÌÒ;?ž	Ž²Üƒ"?c¤
l¢_é?U^<@1'?íEÅOY~?¡ ¬÷
ä%?µ4µÎüª? ÔŽ¸­,4FGL J0221.4+6241e?ÜòDŒ],<?ù—?·¥ôÀ8PÃí*:fÀ:ˆ ¼8*@ò§|Ü@@dß}©y?¹S;€""í?×|CG}m@d@y?ô†@Æï" ¿ã¸Û~@w¿¿¹Ó/<ƒ"ô¿áÃGb• Ž¿é@>aÔ¿í)Ãèø|~¿é+
oÆOTHERSNR3FGL J0224.0+6235HB 3?ÀhºÉÀƒ?wª)±?ëbÌ9X…#?¾ÛxÎ{ï?ÁvËÔǝo?¾@"	¾"q?ÅÚ]Æ´è?Œá<݂š™?ä¦ÓÝyJý?Íuòö*֍?Ö3@ۖO5?Í6´n~?¡­^dIʝ?‹/Q-!ñ?æÛÌ¥ïÉ?¶ûYQqî?ќœš*ç?µq{ž€ž?n¦gËÖ1?Wò0ØH"?àÈHg#?³€ZÕ$¾\?Þ2#&W…V?³w®Išf4FGL J0222.4+6156e?¹Bä9d u?íõ,ÒÆáÑÀ6ã'[·¶»À:;`z"@½…TÖ@v¥xÊí?š±Œ¼ú?л0J@0}?À	oë@âFHä S?À›ïà"?¿Ó5"FK=ì¿ä°>Œ,ɍ¿è*¹¢"ª$¿ì틉5žG¿è=¦S¼?·OTHERsnr3FGL J0223.6+6204W 3?k+PV"?kn"y:?ç³âOA[?ÉÀÐ'ËÉ?ÐaäbÝT?ÈãJ"Ÿ.?q½ógh?y¶Äà¾È_?êÿ!ßvrÏ?¾º×Ë«ñ²?Ãzú™þ™…?¾ œÁ—.Ž? µv†?Œv—'f"ì?ã¦kXÕÑ?º,"àï?Ö°çñ¥?¹+j°[?òw£ú¿?¸@ïJ?ì"+òނ•?¤¾ VÏ?¾ë'%œöÛ?¤LÌ"ü4FGL J0240.5+6113¿ê$â§Cj?ñfþÂ^§À5zÚÿ•wÀ:èâ­â@P'ԅRæ@0Ҁjôk?~>n-bÂK?ÂôæÇIÖ
@=[oâæê…@Vo"w¤¿ÀNÿYfú¿Þ‹É'—½¿äæMà^¿æŸŒAœƒ¿ë¨{Ÿ2µµ¿è,¿0|uOTHERHMB3FGL J0240.5+6113LSI +61 303?ݽá-®V?Ɔ/ñø3"?Æ	ßðf9û?Ãî^ür"?×ÞR&Ÿ4«?Äu ZƬ?¶´¨zAi6?ÌL\íÞð?èî–Â?
?Ô^œ·8?ÀëPºÆO;?Ë:ÀýT	?á¦l§‹?´ñ§8~+w?ËjÑQµ`?²"%˜õó?Íýà|Ôu?±ªª#GÄN>ñx8"½Á>üåü$'?î9r¾Þh?©ÂB¼!?¬f¥ï&á?©Á"'¯›4FGL J0242.6-0000¿è™ºî†ÀI÷%€ÃÿÀ9ÁN_¤À<Iʳ!@æG¤€@'šCㄟ?±ï¥ö,? : ×ùÒ?ë~‰¬¼Œ@Iύ¿âuác\ƪ¿ÝT»ÊàŽ¿çPÝ»1š¿æ?2Ȫ(¿ÒKÃãD2Š¿ïÿŝƒ‰OTHERsbg3FGL J0242.7-0001NGC 1068?ïˆ}õ$ÿ?‡nVaN‰?VPÅÑOÞõ?PœÍ˜V(@?‹jLÄR?†F切ª?ïÏÖ/åñ?!rù›°ì?2³¸ìÈX?I–r›î#?wW¹¬~:b?}'Ç@E~?î¬ÔD8'?•«ÎÝ$Ú?xV»~Aù?o†
­('?¢'äL®¯•?Œ"ba?.ƒ?ï'rÇÝs?rüo•¯â?XÏÜß?LâžÉ¾ð?ˆ·‰R†aY?q—›4FGL J0328.6+5330?êÞįÙTÀ­È"#^À9øxG9zuÀ;£ãŸw)@ùqcÅwC@öVhÂa9?ÈBÎFIm?Öiü¾, @€_&×@
$àŠó?ï­Ä~Ÿ˜6¿¦=žàÅ¿åkB£é~´¿æ–akTâ°¿ïý®KØE§¿íþyzϪOTHERunkNVSS J032847+532859	?¿¿óKcF¾?°–Ç«
yq?·À¸ß"¶"?°C'Ó"8
?éêz£W?¹Ò²µ-r‰?¿·Â{fM=?¶ÊœrµÜâ?¸0M8&Á?·bš;ŸÕ3?éþ	'€?¿d~X¤(?Èþv>0·?£¯Ã0Ö?Ä$bÐ86i?¢0RT»Ü;?äïg®bf9?ª±É0<Ü?ÅÓã&¿(F? –óOæ"ƒ?Ô¨‡ÇãÖ?®ÁFÚ½ ?à6ÃRD?®êÛlErÂ4FGL J0359.7+4445¿ëkÚé'w´À0=µm5À:P "ˆÞ`À;æÝî]@M@H¯å`l|@È!å-ã?»ú# Ä¿©Œסçò?ïùÓ`dĦ?þ"EÇ	"¿êf"¿˜?¿'X¡p—\¿ìÏÀÒÆӿטh û£$¿ë^>¿ƒc!?áÏÐÝӅNOTHERunk1RXS J040006.3+444512?ÛÄ-̏‰‹?ÄL¼Þ?¢N:gG?–:r¸l¾?àùxÁÆÉ?Äeê0"D?áNKtÁBì?ɏM¹6æ?qY¢›x†Š?¸:å3?ÝŒ˜?Èäû["J?åQ¡N+½'?°Àüù`
?¬*}½éÉ?•9à w?Ñ×m¬Á?®|t/ðÙ?é焻ÂÁ?§³kjŠ ?"BßEíî?ƒx_°ñ1?ÅÒ·ø7>?¦ñ€[">l4FGL J0402.5+5402¿ßfš6U/:?ðƒ
%ó¯À:ÔüøÀ;ñ4ØNá@"7ÑÌ?ÿx¹º¡Q?ÊÜ@Þ¡,?‹`Ŭ`àY?¾Ó¯êéÃ@›ØÚ¢"?ÔµŒßvó|?î<xVRó?›PÇåÿ›#¿æ—œ~ÑAQ¿Û0cu^P¿Õ×Ýašy¾OTHERunkTXS 0358+539?âá†HŸ×f?ČjáBÏA?n%(¾µÂ?id<'¥ß?Ú©Bç?āVßȲ2?Õpju҆?ÌwUŋ?yôÀSåP?Œýš˜#?åáv¨nò?ÌT<Ò³¹?æpbØ^"¡?¬‹ä…è(?–Ó@	ê³?~"ýDX±Œ?ѲN²J?«,Úaÿ¿?ç.á²ýzi?°Žnw(?5?~ò=8b?v¥Ù,ѹ?Ñ&s¥¬šK?°¶ûÛéb4FGL J0427.2+5533e?ë5ºOFº@P;£D=GÀ7éè¢ì(³À:Ìûƒ¶@"JjꯋÉ?ùV~AN~é?§þÅdÆ?´Æ´"×j¶@Á`@Q{Œ=e'¿ïÿòɶ—×?ïþÀ//˜t?ÔHk^rÒ¿Æ­ò2ql¿Ôàœbvª¿Õ¥µLOTHERSNR3FGL J0425.8+5600SNR G150.3+04.5?ÛíÄi8Ø÷?É
öè[§s?¥Øãvñà?­v;О'?૏"ôƒ'?ə\k–äÜ?Úþ#?ÐîløÂRg?ÁÙIb©Ó?Ë,¹Tâ&?Ü7`öº?ÏyR€m…?Òt»0á³?°U"-áp?¶6àgMH…? AsŠ?ä,i•}æ?°Õƒ'?ÏKº ´þ?±6µ‹<@?½ayÕë•?¬­…Vîü?ä€ïï]N?¸~´¨‹O4FGL J0427.8-6704¿ìµ¹×ýÑÀCFž<–‰DÀ9{"ÆäÀ<XÚ")@·«N!÷@þxük 
?¬e BÖr?"~­Úï$f?äsÂÚۃI@ïÒ#ù¯Y¿äÂB…5´¿Þ
÷9‡á¿æêL¼ƒ©¿äy'EÖ¤¿ãà>>T#™¿ê˜iñŽOTHERLMB3FGL J0427.9-67041SXPS J042749.2-670434?îó2ý¹"?–€'z,~?a§‹Q–È?X:S+•>Æ?Ÿd®Þ¨ãþ?•á‹n¾X/?ïazÓ'Ñð?—SÃlB?UòÛ˜£*?kh ³ô3?'qwéœ7Ö?•C8µôdà?ì£ôpÉÉ? òÝ,'¸–?''ºÂõa,?'#Ck ?¶–mÈúv?ždqeé¾?ï5{Øè¾?'ÔaÁ…j?'rñ¡Î¼?rÚ)É÷¾?EKj+`»?zîÔ:0ì4FGL J0452.9+5117?Ý»•0Ã=@…‹W"<À9Ò¨Žÿâ¤À;m0•Ê@@ŹE˜›@¸PXÝç§?ÇZSÑä?Ö¥¯Q'Ã@é.Àë­@ݜ²üÂ?ÎK™›òå:¿ÔUäswÇ¿ç-v% Jù¿ëð\>D^T¿ìí8™¤¿ïßøÞ£ŽæOTHERsppSNR G156.2+05.7?Ì®úPi¹I?À›Ï¯SÐ`?ª:âŽÅ? fŽŠvf?ç0ŸÚhÁ?ÁFfÓ:ó—?Ú(pº.{?ʋ3›¢y6?¹ øÖºF?·|_'áÁ?ߏ¾‹"ó?Èõ:){ªT?ßkç
¤ù?±>6j†m?º»`ZÈ4?œõv Ç?ÙåSZͨû?°´_Rî€|?Þ
‹ÀË"º?¨1˜C{ó?ºT½½·û?—Åó£Lœ?Û`DÏÇ	?¨ Ñ»FÉ!4FGL J0500.3+4639e¿ï¦,Zãº@‡?i¢[À8:œÄÞÂÀ:ÊØ£š¤@ïCÿ‰8@:–¹ëH¹?±®+L	?Å2évј@k˽Ù@ÒFö^—¿£—ìÆ<e¿Ôä±z¶Õj¿æ×2ƒ2¥¿ä€µ¿ë%F Û¿éøDŸÂ'­OTHERSNR2FGL J0503.2+4643HB 9?ž^Ï8å?–kDS¿Á.?Æý9¡•?¾k_
"î?éM»ӗX?¿²ç2Í?Á!ÐË|k€?Ћ$ð˜Ÿ?ßEç#"Ä&?ÐÁ¼œàx?Ø)0w?Í:‹¾fk?Îîå—}+I?­qÒßëu?ÍÂri?®ÀÿjÌp?àÓªØÚè?²@2³c†ú?Á3 :Ç~þ?¥UJoB?Ä>ËèìÂy?¯¿{jnM9?æ£d÷ï¢?¸ZK€ä2–4FGL J0517.9+5030¿Õ*Kƒ8@NÏ~Wô´À;í$[)À<uŽÀøƒ4@×̃%äÁ?úÒ
#opÑ?ærÙ;p—?ç©8¨½ùË@;šÅ都?þGÙbÝDê¿ïüD=é?ïþašNË?¿ãÇ}Øró¿Ñ}Nñݨ¿ìÄÝëAú¿º_Êø®OTHERsppSNR G159.6+07.3?å4uÝ!šñ?À¾=æY?«3#°‰û?£&ÐAû‡?Ò%máF¸ß?À¦>ùÂ?ÞmAžî•ß?ÑMîcáJ?½É%_5@?Ö8¤š?Ú u	D?Î*ù
#uÆ?çëŠÆ=@?§ÿ=?忖?²éŽÕ/r)?˜…¹E°?ÆÝ
|sF{?£Š›»E¸?ç¹inø?µ¸K"U˜?¤7J•Šb?ªÝÆ·‰ñ?Ì΢M‰?³2ª¡¯µ'4FGL J0519.9-6845e¿ïñ¶°À@±'¡ ÏÀ6îñ<îØÀ:\pšœÎØ@C¡lv˹@Z5þ¿Ž ?˜Óy—ϼ?ż°µj¬@,H2ËŸ@5ëq…¿À²ŒÙÔG¿ÒÄË¡~•\¿âóó¢y'¿äªúêíID¿êWºÁÝZ¿ÎH"•sOTHERGAL3FGL J0526.6-6825eLMC?£¶ôSd«~?œÂ&"¯(f?ÅƨÙÅ}?À¹7 ŽÄ¡?é~_"Cé?Áx‰£ó7Ž?˜6ˆ³•Q ?¢6üÉðy‰?í݋Qeâ©?­úymÔù?¦×,ä?¤_
¾ú?ŎǵE—?ª)£¾âçl?ÔJØ¡ïÖr?³M˜,-Tß?àw
=Ãa?´")Y-I7?TÀÓKpÆs?Jp+T™v?àËÞÙ¢c¾?¾`9%šf?ÞSyoǾ?¾a
‡P`Â4FGL J0521.2+1637?Þ¥©ª*WåÀ&©O‡À:–E"I$À<!]×MY@ëÉa2tò?ø~Ûrýœ?؃b¯É?ïNH,¿{«?ÿú"5¬Š7@ŒÕ»Þ¾?êfÆ"Ž A¿èðaՈ¿Õ@˜Á­^ó¿àåQÉ oâ¿é*‹"ÞQ¿â9¾'‡.]OTHERcss3C 138?íÎXµ#y?µ{¸Y:?}RÔaApB?±bh	¼¹?µ|_ôBÍ5?´æΡ|'¦?íʈgés?·Šâ®Ûš¶?"ß~}õ)i?¢XžB ?®™áñÎv?³U.ÎÓ?ê1§lŒ`‹?¦àQsÃûÔ?¦üÜ}…ƒÜ?•%:Ù,'?Áz+.mÙ?¢SÞpP'£?ìm ™˜[½?¥Š¸ÏœP*?z¸¯JÂ?rèã+jX?ºëpAx1?¤ðVÌg4FGL J0523.3-2527¿ÚÛL
ìõÀ=Ô2‡;ÉÀ9$éºC]MÀ<4x'@>^çÁð¦?ú[™hò1á?±
Á$"8?ÛE"~°	@)
fðÏáT?÷¡º¢¨¶î¿Í÷Pƒûø‰?£Drö—¡r¿ÔB©Þ5Tö¿âo9©nù³¿í隁öæ¿ïÿó5bBOTHERbin3FGL J0523.3-2528CRTS J052316.9-252737?–Ã/­îéy?–M"Sí‰$?íÛ@ÿ§9•?±;¯jÛk6?¦êX."ñð?©›TÌ	_?"™p•qt?—wÀz€P–?íò‹šAk?¯ïjiõ˜Ð?¦Š—'0v?©¹ý{tB?šç¦žÚ]
?iù踾U?ìïªM'?›µOñk?±Èŏ^ü%?•"G7RN?~1tóRà8?q"fÃá	(?ì
¥O‹þ?©ýrOæ G?½ÇÀNr	?¨éÑڇ4FGL J0524.4-2413?çø‹ ˜Í}À=3ÚÄç%À:©VI¸±À<:Ȇìî«@R`¤.É@`Eºõ4?Àuf3¦¿´ì×?}ªŒ?íB–%œr@¯p¢)‹¿Õ|qÀŒ¢¿èÒ±þ•FÏ¿äö©Àd¿êáÏ=jn´¿Üz¡Ü´ "¿ïÿ⾦™\OTHERglcNGC 1904?ïÞJ°"~?ië˜##P?R=n®"Å:?LZ[%#?h—Aø[Û?eÄzK'µs?ï'oS@|"?†9òÌ¼?=™K "²?T°?°ùÒ*?Š·`ÖÜ:ž?…Àvðóv?îBO׎æ?OÄ@Îå?}|Ýñm?m½*ÎÙ¼?¨+—{Co?Œ%îíÌFû?ïL¥Ö©‡C?|e<¹á?X({g$[?QéÒôç€?"è½t]%7?{ºì<Dü4FGL J0524.7+4824¿Ú£èPû‰è@6D#EfÀ;š%FáeáÀ=G'u¦@ úèóžó¡?ý}ÒÉfÿ?ÛD^ÞÜ?ï¦jÍÔ3É@s''%Î@Ÿµ§ís¿éÆl`{jÚ¿ïÿâ¾÷!?ïþFŒ¬KM¿}87Sÿ0¢¿ì=˨	žå¿ïÿúâôOTHERsppSNR G159.6+07.3?ë-T(ÌÝ£?Â
¸.æ¬É?–½	Fÿ¹(?"rY€#?Às3ì'O?Á¤Ö¡ôe?Úàæζ?р^Ié;ø?ÅãŠ:áJ?É.ˆ¡¡[û?Ú.5ûÁ>I?ÎÏXjC¬b?èŒ
¯çi›?©z…¡Ók¶?²µ-pÐÒ?›iiAìÿ?Äu>¸)ñ)?£ðwî9÷?çÐ:ÃeÓ?¼UÞÝ ­#?™$P?¹§ÉÓ?¼M7áÚ¨Ç?®z-)G4FGL J0524.8-6938¿è_†³bîbÀ@f>lLYuÀ:¯wOµóÀ<>¼(@ P&'º'.@#\ƪsÜ?Ƌ«Dfâ7¿q;ÞPÎg?»7…RdѼ@sÎáÏé7?îF7òµ•¿çM|5Om¿ëøýbô´¿×̤½äý¿Î±ZÖeQé¿ãòEÍiª¿OTHERsnr3FGL J0524.5-6937LMC SNR N 132D?íC*+8J2?¬	¾
1œ??g5'vtÁ_?`èÂäSÕ?µ-Šs?«"6J´?ï'I·lO?šù®©ê"1?WØT'·?jîR¦øþ?™¥‡
J£?™'¼WÅ­c?ì
¾ñC?¢Çïy*jþ?ˆAÒzO?r	÷Õ¥H?½~9Ñ¡2X?¡¨}vml¬?ê]›ßè:?¤"ÐW?mY{f‰†?b˜"D»	*?Æ,q{ ?£ð]}.'4FGL J0526.7+4254¿î_õç€á@<"Þ ²'À9¶5•
BßÀ;‰Ì·ÔD@r§qsŠ¼@'»0Ã?À=̀{æU?ÎÎ81ʨ@	Š]ò#žk?ûR-ÝZ¿ã>|b&:ҿфîê3¿çžfB)EI¿æ'¿BJ¨E¿ïþ&@Üi"¿ïÿ‡ÕK÷OOTHERsnr3FGL J0526.0+4253SNR G166.0+04.3?Ùÿ°·ö?Å©'Û™î?¿5ª;vò?´¬•´´ü¥?Þ2åiƒO?ŗP/¬âp?Ép‹W*-É?Ã'R]RS?Îxqf6\?Å"¹Õ?â#¿
Ûæö?É{ŠOpö?ؗÏ*³v?¯Ûý!?Æ5¬³2•‡?¦È:<å$Å?ÜMZ|RÆ?¬])ùÐ>?Ñ÷QÆÇÝ,?®¢x>?÷?ÇRB
D©?¯¢øð¤v)?á/ÆyXÀA?·z7§¢¤4FGL J0528.3+1817?ŽÿÛ$ÐÛÀ"zd×ñÀ;
mzVÞ3À<bً÷ðg@""¦ö¤b?ù£l-Î?ÒêsÜp®¿?Ó<'`
ª@Å@Ìxé÷@Ug"xû¿¿ïÿúŒ"¸'¿ïϯ l²?ïÿõMõVY?_³nØ¿ÇÔñžé9À¿é÷ƒŸ‡DWOTHERunk3FGL J0528.3+18151RXS J052829.6+181657?èêdº,Iœ?Àò­Å(Ü?qé³–Yž?ž²µS¨ˆ?ËÇ$)²&Æ?À¯üÝ"7?âÏåœÏ¶¹?ËìNL¤"F?ešÐ¹!'?vJ<ƒUœ'?Ú4ÿ$îbK?ËÛ®¬Pt"?èHJ(ÂÒ?¬òQ‹·¢?—oú´¤n?"LÎä\?Ëí)`^`(?ªâØݯ?éç1È.¿v?¯qyÀE'Ž?oãQtZæ?m­WW½®!?Ç㫙tè¼?¯VËûރU4FGL J0533.5+1449¿ß­¤%öÀ#•ÿ'+¾ËÀ:æí1Ç"iÀ<8|É:s@!M³ûo¢z?ø\'þ!?Ôèî Y'Â?Ùâwä"?þ ©¨ÛUý@_~ptZ¿çĀ}hák¿ìÃÏ,ù]O¿î—àÓ¿Û?èÙ¿y}¿æ©³ÊG¿ÐWÍÜÂ8IOTHERunk1RXS J053336.0+145115?ç t—;w?ÃB}¯n˒?uMš"ïba?q7è…3ô(?Ðiàhþ‡?Ã'WŒ±Í?çÊ9î©÷?ʁ¬nvY?j`â+Ø~Z?†ê'öÜ)?Ð6ÌÊû?Êh½«
"
?éð@N<?­3Ñ1E½"?›èxß?‰¡¶"i?Èk0­}Ë1?ª6nþ]‹Ç?ìЬó8?°dn-ù^m?x3ùø]\Ò?‡* |b"?½Þ:øáPi?°Y¯ûÀ)4FGL J0534.5+2201s¿æDùQ:/QÀ 6m
JÀ6"UõÕړÀ8{•É*€Ý@e
'àÃ@
Ÿ²$ªÚ4?Ð^beOæ?åLïg+ˆD?÷±ÇÞP'Ï@ î'š!¿ãq9"Ÿ"•¿í¦È •¡½¿ï·Á½ob¿ê tοêÑ¢ßé_*¿ï
²¢\·OTHERPWN3FGL J0534.5+2201sCrab Nebula?Ãm˜j"+
?ȁæ˜õ«?…K™ºýc?µlÍßCÅH?êÏk~rÕG?Ê)dÁe,?îz‡(bC·?¹ƒ,õd?y‰çËff?¨"¯Jg?¥&P€kײ?µ™7&{|?ÜK3­Ùº?³»ij¯› ?½}‹´'?¤JqVe	?ÜUŠ¬/9!?³FBçö#?êÿ¡·ÐwŒ?ÆÏ3XM™?'Ü°Gô©?+d1'B†i?Ãûô¬\U?Æ۟½‰4FGL J0535.2-6736?їޒ‹ÍÀ@óGÀ9[‹]–´À;«qóbbÌ@<°®;Ž@ÅÊz5˜?µ	5'?ÈŸ‰ɺ@d:æ…Û?ý˜ä«㣿©òÕÊø6]¿ç$²1@ì¿æ¥Õ|ž·¿ëP™àç6¿ìC‡¿&›ö¿ï^²"&›uOTHERHMBLMC P3?àâxÊòí?Ä6¼ÄoCø?Êi4ñõ£<?¼¨Æ¸ËÏM?Ñsñ þ‡?ÁºÍ{Øq?ÖOÍÊB?ÇÐ1É?Þ®•8·µH?Ê«m#çä?ƹôið?·&b@•J?ã^­õ˜<?¯CaR»?Ââs–CÕÎ?¦º'gq?Ϣԓ[¹D?¨kõH?ÓÛ¹¤åRò?©8ýPM]?Ô漫ET÷?³ÞÌ|l06?×=‰¯ÕX?°—_Ë顸4FGL J0537.8-6909¿ïõ!È°;$À?¾)Çy¦µÀ8ÿ[zz¢À;b8¦@!&±ú8•É@Dº"»äG?®!ý"L}~¿œÝÑ_Œ?òˆêõ¬À?þk,kÃÈl¿ïü,k˜ÕN?ïF2nè¿ÛU^–cY¿â/Ljp|¿åðª!§µ¿È÷gjW¿OTHERpwn0FGL J0538.4-6856N 157B?ísÂfï?¬èpo¬—?k4š8?h%Rª?³ˆJSâŽ?¬NiyZã!?ìXC§/H1?¾Îm–}?£[©'¾ÓÌ?³'™D9?³2¦T™?±ÁG§".?á^¬çC?²¥ÈƀÌ?£°ûêÃÿ*?¬kÞMé?Ú̆´¦}'?±–E¡T9\?ÚÞò–c¯?³G¥?¤óð?¹áE˜¬ ?¤úÇËj\ö?ßuϧ>"I?´p§uDEc4FGL J0540.3+2756e¿ØúLö‰¿÷ÿ@wÏDÀ7˜€dÀ:nÔw»ù@@ƒw3@$Ñ~uY?©f\^rT?¿úBPÝh&@•èO	R?þ`4:Å"ß¿ä7Ö ²Q¿Ò¯&ÿHJ¿ÞÐÏ%l¡¿âí±^\Vÿæ²Ô~«¿å¬Xž&ÇOTHERSNR3FGL J0540.3+2756eSim 147?'e1-h†=?‹IOlN?…÷ÀK?ˆzåv…€?ï÷t`GÁ?•gÒq?¶ùnrØ?¹Ñ
ëÒ4¦?Ò]-½Ñ"ƒ?É놦[ªŠ?ä)óHÛ<?ÊqNêՈÊ?ÄÛ¶ÚsŸÀ?¨©5Åo¤?ºXrR+q?ŸÞ÷•£×­?ç~	XÒ¢?¬'&"h4›?³°®¾N¼Œ?£ökfúÌ?ºÐ¯ó‰é?¯Ëøá'»d?ê/Ô)Ò·1?¸‹1Àøg4FGL J0608.6+1149¿íhtÛʸÀEà.©`·À:5.¬À;´¦Hԅ(@s¿®+L	@M»$-ܲ?Á™UQF¿›'ý\ÑV
?Ú³Z€)0%@eZwÅ´¿ßWú'ص8¿á˜f~9@é¿ê˜!"¥>¿×mÁðzÒ¿å'U¢ÉÄ¿ÛöUDz±™OTHERunkNVSS J060835+114942?ëÊ%;ÁÕ?²£cIÑj?o©É×^…å?n>ÁÚÈ5×?ÀXÄk³~–?²xw–ôxQ?å`‹Ð(?õè1DÏâ?PÜâØ…"?g6ì4•}?Õ¾b‡J?çã‡ï²?ê`B?ͯã?¨óÎk" ?Š>Ç~|°?w5ie½3?ÄÝcQX¨?§œs¸}?ë*—Dÿ¡?žË­këÎb?n¥üÃ0?]ð ›û2?ÂÛy¼m?ž¸ÛBU-±4FGL J0608.8+2034c?ÉJ…ñWVå?֒*߈'À9Û©ßaûÀ:ɛëƒq9@™ðX˜—@"‡vf?Æ~ÿyó6?ÆûBÁp£+@0¦ždÚu@@®pì&¿ïÃvõ׈?ïÊÁ$"8¿èË[þ®qB¿åµ¦	êd¿ê°Ì†Uï÷¿ïÿÿ&¦³OTHERunk2FGL J0608.3+2037NVSS J060900+203746$?Ñt;—í?¹Ãº´t=?Î?·SÇ6d?¿Dûóꥪ?ßkèÆÌà?Áñ§§‹q‡?­òyËÉÆÂ?²¸2p&ç?˅.tzd'?Åìax¬í1?ç?ŒÆ$Êp?Ç­ß#	?łݻPÉÝ?£ãjÖØú?öEz'v?£zî¤â5?å×ÚÿÍC«?¨ø͝| Þ?¹ÈA²ž˜?—®-UÝK?ɀ{èè´È?­¹ëJL?æfØÏrü?­Î‡žP44FGL J0617.2+2234e?ë>éÆò\@DÚ`3FÀ5†õ)iÀ9ƒ~mÄ(¹@ —r،I@ýo¿«|?‹¼ê	Q@?À>¯þŠßí@6ú;šàÁ@$&žü?îxˆr)é¿ÐPF~êkÄ¿á_eÁ$øÞ¿áÅÞ,ñ{¿æ*Þ)£¿åWǂ
0ÛOTHERSNR3FGL J0617.2+2234eIC 443?¯‹?¨¾u¤?«£ÀÎNÉ?Áœâ+zQ?ÈlrÖRrå?é €©:?Éú"ØO2Ñ?'­¬Oe'Å?³ÜÅ¬[?駞õ)RŠ?ϔºúì`?ÇΡnà?ÌØ8Êþ?Ä8ÒcYç?±áÉÇõê[?½ö:ÿkJ{?§9Óؒ?ç3<37?µ»'ÄdÌå>ȱj)d>ÏÒÒ´¸äŠ?ìmGŒË?µ@#%œ?¿<d`'n±?µ?ù/G ½4FGL J0618.1+7819¿ê¬4M(kž@8ݘ9GIkÀ;#''Œ6À<ÎYáÒ@Lû°>@D.ÛµÜ?ÀY3¢ï®¤¿µ;Šo°*?ð¦ªú-´?ô'ëí¤]Ã?ë8Åû!?¢‰grU¿å]Ðà؝f¿ÓÛ\Ý{›­¿ìÛ~WžÍ?Øý¥²¬OTHERsbg3FGL J0618.0+7819NGC 2146?î9]9Ä_ß?§YޜS7ô?œ\œ&/S‹?›_›øFÌ?œw¼¡D°?š…¤þ$Éæ?ív­^+ö?²ú¿"²O5?èéæ@R_?§'ЃxÎñ?°r~‹²?§0Ôå6:?ìÃ	äŽ?ž=âÊik?—t1f
??‰"⺨ç?´','
Q?™*ÒFx?é*%)n´¯?ªéxž\?»€2AºÆ?¦5eê:z?».¤ssŸ½?£!¢àwh4FGL J0632.8+0550¿ÄÀ¬ÖÀÊ¿÷*°ãb:ˆÀ:b›!YÀ:ý³çùxý@!Ï¿4ïc@%!š"{$?À'¬î
46¿¸?³ÊnK@üR`õä@>bq`?í²µ)B©¿åèÍÿ|Í[¿í̌€V|Ž¿Ù÷›Â響à³Ü:þُ¿ß÷ë>Qõ@OTHERhmbHESS J0632+057?§s™ùâG?£Ö5
ú,?rçä''?x̃"ÿÍÝ?îhZė]Ž?¤í ¢,ë?¾aUJá7?¼Wއ¿	u?XÛýZŠ?žˆc*[º?ë¾qæ®nõ?¼‹ªÓ" §?ѽµu?xV?©,w¬;K?¦ã®œP–?‹Ïu2Pï?å¹
v~Ì?¨Òã€}«?«žÑ~®A? J!À<M«?|@ý`OèÍ?}y&žË'?î
¤'uJ? ç`¸ÎôV4FGL J0634.2+0436e?ì†÷Xű¿û4ÂI¼´À7cx WÀ:]I.G;(@	G&…%@Ôó\ƒŽ•?§'/ÞêÝ?ͯº'ÈFÖ@"×\l¡?øá@âV¿Ô(þ;"»f¿Î…:¼êV ¿â†HÿxE·¿ç"O…yQ¿åYÏ^ø]õ¿èxŸN€ÌOTHERsnr3FGL J0634.1+0424Rosette?Š
ΜSû›?€ò•9מ?ʃôªêœ?ãÃ_X¿á?èö˚Óþ¬?ÃÑõhd?‰d:køb?'W>ç?é/jÔPµ?Âúó" 
?ɬ
Û%¥?©˜5‰.m?´>Á¶Xƒ?žñ5
F†?Õ­W´Iʺ?µK"O\$/?â¡{ï
A?´ñÇ%¥Ê$?tžx³|™…?búPqðÙ?Ý­º*¸?Ádü÷?áPì1"q?ÁoÌæ="4FGL J0639.4+0655e¿×bN
?àŸS À7 /^'\ŽÀ9À¡²lÏ6@o½fþ;Û@a&Á4é?´b_£ÿ?ÏÆæxFä@X_^4h½@@í°òý?ïÚ䜸2¿× (ú¿åcÀEç¿äŠ]âsA¿ëÉF/9Ä¿æJe~ßÙðOTHERSNR3FGL J0640.9+0752Monoceros?f>×x¢ª?]‹'GiÛï?²,ò0zþö?¯ÜEüˆÃ9?í¤#ž'€?°
)FÔ?•Ñ>wƒE? iV¬%—)?ä3¯¶ø66?ʌ¢`0>?ÖG~(a?ɽVõ÷ƒ?·R˜;éï?¢n×þ—Œ<?ّ®WW
r?µ½ƒUP,?àLÕÄlü
?µ@=¢ÃD?}ü+<¼¿?užš#ďA?À"€Géíî?ºŸ#­m'?ë»fï¯?»ÕA+>•M4FGL J0647.7+0031¿snŒ"™¿âN»ßê‹ÐÀ9p°;œŽAÀ;X4Ò@ŸÕŒcûþ@ÀùÅS[È?⡟øXkÒ?ÃÆe¿øS
?ÿ€–"TÜ@‡f$w-´?ïÿhJí¿º¯÷¤ç«¿éºÄöJ¿êÒêRï'¿ä

ù½Ç¿áÓàx"OTHERspp3FGL J0647.6+0032SNR G213.0-00.6?Ü+C•£†?ÆksËÚ?'TF#Š™=?•-]­èŒ?áW¼r?ƍ©Ã~Y?ÔUÛB*³é?ǼµqØ8?–§df0U?¬p¡ìK?å×;¹%á?ÇÆê]1?ظ"]2?°w#ýÀ'?´Ñ
ìW?š;ÐG)}?á	¼Îމg?¯1ÍîA‹?äÂÙ'?¶ŠDvó~?'=bBÙ?˜—¹ü
?ÕW1€(àÍ?¶|«7ðoã4FGL J0650.6+2055?çø×:ËJ@"h/"BAÄÀ9æۚÅé"À< öðŒÅ@ úe	.O?û

jKÎ5?¼a%r†Û?³d' +C¦?ûVʗhfò@VX§6?ïðHgwÞ^¿æ¨
/"k'¿Ó6@®ÆÒ¿Öµ@S­&>¿ÖasÕB<¿Þ·a`m("OTHERunk3FGL J0650.5+2055NVSS J065035+205556?è«îs‰æ?¼ÄäÒ?€q¾toÍ?vÒ§*s ?ÌI7²J'l?¼oƒ""Ó?⏒•ü&?ɬ´–)YÂ?x>°`Å?"6%ãô²?ÚâĝF1?ɀËM¡R?éÕ}–ó±I?£Ÿ¢Ò§
?Ò ¬ÊFx?xˆ3òA]¦?Ƭç™d–q?¢kK'øå?ênÔ4':÷?›á‰<mL?t·«èù?x	]5«Ñ?ÄB˜m—?šÞv°`G'4FGL J0709.7-3009¿ïë½>ÿ"À#J½ÂmÎ:À:—¥ßøù|À<b+¡ƒs@ Šý?ÿGKƒŒ?ÁY:?w9gïlMË?¹Q8½òÐ~@F¸4Õ?ïÿК·¦Ë¿éiüp¿Ô/(âwXý¿ãŽþ "of¿ÕŸ{¿ßއŸÇ8OTHERunk1RXS J070947.9-300901?ídœ/4?¯Çt?V
ñ?Qøoùœ¯?´‡v¿'N¡?¯vÛÞ>i§?ç<oë±j?Ç¿_'àµý?RŒv82Ÿ?l£9}½%Í?Ñup©ðjf?Ǫ"Yç@?ë¢à™*·?£Ï¾¹À"?LB"*×Z?mæ0÷pZ?À_»¥X§«?£Ìq‡#?íª×l2?™æ/&læ?d	(ÿ?T7…W?²þ'Ë?´'tX	4FGL J0744.0-2525¿ëJ¯×|0Ü¿ç§ÃÉfÀ8Ï}ÓjuÀÀ;z鳍a@Š9-s*Å@¡½aõ¾^?³ÝLvѵ?Úͳ\cX?@#HÈ/ù?ÿŸlÊX©9?äJSá)¿ÓI }8é¿ÜY"åO¥…¿åßÖÊ|t¿ð?ïÿÑqw;¡OTHERbin3FGL J0744.1-25231FGL J0744.1-2523?†[EØ8g?†<é3¶Í¨?늨ղËÞ?À:†?¶?Ào¨XwM?¿.n¬ßíŠ?•lá3jç?¥"•µv‹?ç,jAÒc{?ÈܘÐÐ$ñ?ÐU¤®H]?Ç'—äG"ü?"ànýFF<?……~ÃÔ?ëà¼‰,!?¡Äwó±Æ?»Ç~\e
c?Ÿøf£é?Š‹Þï·?vÅOFa?å£<X=L6?¹LVßÐÓø?Óå(X¯s?¸çŠÜúç4FGL J0809.5-4714?ØéՉðëÀd]wª\À:
%ÍïâÀ;ÏVØSéŒ@Á…§IZ'@*N뒋?Ã'CeÛQ?ºH"Cnj?õS½vd?ýŖ­V¿ÙT:귙¿×ä[Ê+1Ý¿çý'1ÆK©¿åÈØ\œ8¿ãف±E‡Ê¿ïÿîÝÃÀ	OTHERunkGamma02 Velorum?ä<KdD3±?ÀÔF÷ówt?‰•ÃØç?|'çə?Ö¿‰X؏?ÀÔ±2žæY?ᕦࢠ?ÉÞؽã¿ó?}ïêºT‰ê?"ž"m¦Ê?Ü\ò"Ò¡š?ÉÝa`(f¿?卟s
?ªÍW-Œ*?§ãF1éb?ŠIk¡µ(ì?Ò"±$ÀÓ?¨WÓ½êG|?æç–íªJ›?¤a‡Èh??¢†ƒ¢"|h?‡]Zàl\³?ÏÀ`±¶x?£ß?è6s4FGL J0816.0-2342?ÍNâÏv(@o4þåMÍÀ:SŠ ÒHÀ;Þ€@J‹¿f\Ö@–Ÿ¸g?ШÄûb?Ó.ƒ€Óz@¡zSƒ5@ˆ`â¿ßRBã)…Š¿ç±/Lô¥Y¿èђ>†x€¿ï[nÎ?¿ïu'>³D¿ïªáö)½iOTHERunkAT20G J081524-233846?èw ZKÕ?Àȵi¯™¼?£ÚJ©MH?j~`Êm¢?É-fÔC~©?¾Ñ/
1½m?ÛnÂѧ?Ëq9ËóþÃ?¹Ûbô8?¸Sˆ:†Šï?ÞlËû՛â?ËےZPo?áça§¿ÛÀ?°tŸÃ®C?Á$ô¡›`?¡\ƒ¨?ӟ:¶/zÐ?ªhÿ@›?á¶Ãg¼£P?®'›‹¯V?º°ët­Já?¢ºÃó×Ð?Õæ>S[f¨?­ì–±U¨³4FGL J0819.5-3439¿Õ9–Т«w?ëû=#JÀ9ÕÊÛ[	À;zºÖ*D@ég)ÚÄÝ@":ÚÇa?ÎTð]-Ù?Ø"Ÿ€&@þ'Z·Ü{@¼L0Z;?ëˆÒ!Š_¿Õ(,ÚSž
¿êÒiY_í¦¿èÓÀ§$œ—¿ïþP¤]B¿¤­ÝTOTHERunkNVSS J081945-344215?Ö1-<î?ÁØÀ'Ÿ]?°B"õeFL?¨§…O÷í0?âßÃMK¿?ÂQéŠÝbY?Ø¿»c(þÅ?ї,ê7?·J?ӑO‹?ºíë"Œö?à¶ÚSùV¬?Ѧšß¨O×?Ԋܮ‰á-?¯¿hǨǤ?Á£I€'s?Ÿ4•Dʓ2?áQ¿Hšr¦?°ŸXT¬5Ù?ÕÕh_ïï{?¨ä"üjÙo?Å5š•Â¶‹?£jgÉ!µ±?ߏÊU.µA?¯€O–W›š4FGL J0822.1-4253e¿ìè»Z+À
þ€{»bAÀ7M—üágÀ:ª}ÞR0N@ƒexy?þ"Á-\Y?Ñ÷À&²X?¹Í½7®m@Ìx £
·@XðCõMJ¿Åi€Íú¿Ògáæl¿Þ=êg9 ¿Ü­¤"r¹¿äŠS«x¿.¿âgk*NOTHERSNR3FGL J0822.6-4250ePuppis A?ȧØê3
?¹NK1ë?ª0œÊSõd?¢ð°‡.l?è2ÿøÓóç?»›ÂWßc?ÀÜÓ5¶n?Ɯȱ¦e?Ú>Ž"ô{â?Ñ`dS!ðí?ÝSgp¨ç?Íb8³HP?ÏxÕ|¬Ûõ?°m-Åfr?Ã7
*aƒ€?¦¨ì§8˜Q?ãTV<h"?³kT¡ ¯?³E'–ÕO4?›&¹ " ?Í&h¤¢?µw§Å ‹?æM³£üÐ?¸$CÓ=4FGL J0833.1-4511e?ëa…DçªÀÙ0¾
í)À6¿Þ^sSÀ9BY`Äeö@!ägÀ`@QŠ¡¯Ñ?¦¤©;?¡ÙÖ~/
'?ô,Áÿê1@ãhšž&q?æU€e.?ҩ… ¿à8¸¾M<¿Þ¾u5¬¿ç=ñ7¿âµÚPp[OTHERPWN3FGL J0833.1-4511eVela X?;u&+«á?Ã(çïÑ?XÓ€/Æp?e¦É\´DÛ?ïqºÒŽŠ½?m¢K4Ë?ÈniÒ5é%?ʁ@ìíÞ?Á‹¢û?ÈøI"ô™¦?偟b³Àñ?Î;CE|ö?¿RÌöw>!?¨ÄÂIñA?«øBã/
Ž?—¯>ç?êV"2þ'"?ªÒRôB'?ŒÐ|W§?'Òe¶g†?²¼tg•…?£‡w#@ŽŠ?í$͒²'?¤ÊÿÈè+Þ4FGL J0838.7-2827?çMàØ8ç@=5¤&»À9"©¥€W©À<pÛs@Í(+˜4??þv9ïå×?³€šëSK?Ó3\£Äì@ïbùÊ\@$ïªGfÇ?ïõT9¿¯ÏÛ Ñ¿Ü{ÔA‹:±¿ÞœÆtÃ÷;¿í­òˆH8¿ïâ."'AÜOTHERbin3FGL J0838.8-2829XMMU J083850.3-282756?ˆÃq*¯ë¤?[Aw¯§#?í¨¦­¦X?©NIÙ=X"?¯D¸Úë‰?§`³¿?£e"¬:7?©;sÔ³÷?è:Æ£¯™?Çù)ܨ$?Ê;€p^3?ƺ-©/Âï?«#]cb‰?BŠ'X?ë]‡b]—û?¥-y¶ú}?·';‹é?™û¯¼Epë?½G]³ÃíC?ëä³)ìë?æ)…+*N·?±+Pì+¼?ȶ<yt΅?©@Â'<4FGL J0851.9-4620e¿æÚÉHº{¿ó·þ½à¡À6Õ6$;JÀ:p³"&k@!²KH¨»K?üßѧ' Ö?'Jf¢î¤Z¿"¿g€å?ûÄ¿9aK@:=,0_™?ï	H]ç¼½¿Ö©CEO¿âm)c¦˜†¿Ûd`½/þ¿Û±€@,?ú¿È ƒxÅäOTHERSNR3FGL J0852.7-4631eRX J0852.0-4622?´"0R‹!?«¸ëàtY2?vb‰ÿîè?xædE*6Û?í@´á®ÃÔ?­°"£'k?ÂMe¡ô+E?ÃæZö…?¦Þl8Z¶?³FŒv"X
?éþ¿Õßo"?ņ0{«Š?ĕ5Dù†@?«SÀÇ<H•?¥0g•È??Úݙ?釬5e€?¬Ö´5h?ÄX¶ìb™¯?³PvQy¬?À!؏GË?±C®pë	9?æárNÇ¢?¶ó~[òï©4FGL J0852.5-3123¿îƒ$Bˆp@ ½óùa€NÀ;,%5À<ƒ·'¸¬"@">NÃ9%?ö.­ýÔ¬•?ÑàÙ^«‡?ÏÈžžç?ôŠB®Ñ9C@2õ#Øø)?ïf¿2Zp¿ïÿQ^ÂX*?ïüÉÚ¨X¿Ùoß¡eÀÏ¿Èø»h {¿Ð$—Žý^OTHERunkNVSS J085238-312331?êÍð(¥ýÚ?¹yóÕ\‹?c9J±ô³?_ÎàK­¡?Ä{êx=@Ê?¹?¡éxÿÖ?à·Vã/?ÈÏ	N•?Š"°¼Ç?"Ë7GSá?ßn}l¬³»?ÈhXÍÈ,‹?é:¼9[¹2?¦0ŒtÂ?±}æŸ'î?x6
ÌÈÑÝ?É9÷<'(·?¥+ð—ŸÂÍ?ê"61m?­¸¢¯ˆÆq?^[tìB¥~?ZÈ|x¿?Ç:qaÆX?­¼0V/['4FGL J0858.0-3130¿Ûß÷ªy™@"dj ‡ÊdÀ:^Y­ñ?sÀ<6×%ì"Ó@!±Ÿˆñ֝?úÍwҟt¥?ÃñîšQûJ?·ø™Àl''?öf2ƒ
@!Uå?ïâO`:}T¿ìénù²Þå?'îSžýJˆ¿Ñ«ýI2¿Ôž[JS‹¿ØUd.(OTHERunk3FGL J0858.1-3130NVSS J085802-313040?äә¿nº·?Ä35óœ>³?^ƒ«&T%l?Q"ys[¥S?Ö:HÕü6m?Ä0ÍZ4~!?âqüVïÇÁ?Ê'×ùøE?msNþf?zÉFüÃ<õ?Úá µþs±?ÊÐÆ¢bv?é{øz™x?«Ê=»é¿ñ?'ÆâgcKð?l¡Ì
öÞe?Èç)÷Ÿef?«8m•ÕT?ëR`••‡è?œ2™ ÷?qüóƒp?a՝ܱ"?Â&–	DI?œ,gLD­4FGL J0904.7-4908c?íŽÊí	êK¿öú@óæJÀ8ÖÞZ"ÊÀ:Z¿»lR9@\´5ý@	STÛúg:?Ð@rM'À?ß݊àY@ŸÖjÛ@@j>NX(¿ìîàwW?ÛO®~ƒÄ¿ëU£ ƒ˜¦¿êÐäôá¾Ì¿êž–Xœy¿ïÿG]â‰MOTHERunk3FGL J0905.6-49171RXS J090505.3-4903244?±Wnç=ƒÕ?´Y‹"ÒѦ?¡'n7¿?£ˆrNXø?ìÃ0©ñl	?¹¢ô<|k?¯4Îßqþ?µц
Ÿ—?Õ…¸0'Ñ?͇ìø願?ãˆð5ð¦W?ÍØó~z?ÁG2þ!é?£¼Éò@'E?Ä~ª‰'`?¥d®«ê?æ­Ð^.?¬'ߏtï?",LŸ€úý?~dRç°Ú?Ø  œúîX?¸Sùþ8¦?ãNL†€ü?·û5Ó]4FGL J0910.0+4257¿åpîÈ}»@EvFbºà;À:i—Sn<À<{8bG@è!©s~@<¡pþp?ÎêÒñ±‰?ÓЧ¸@MÎ@5@%Nn@·'ŒYë?íݻŽZv¿äðÄ"ð¿äÅõãF‹Ö¿ìÒÏæ\ÀË¿ïì¿EûŒÔ?ï¦ë\ÕOTHERcss3C 216?ë"Ôc›?µñÚä²("?'è㨯Ä5?Œ¯"§mù)?¾åHr·2?´×p ?êØò!Ve??½éLp•)?®'â"Ù¸?µg#C1?¹öý«_ô§?±Ÿ[¸g–'?éÃSDcF?©]"鵈c?°ØŤŽ?˜ÊfÎm§?À†±‹æN?¢…Âï?ì.˜î+uƒ?¤0.Ƒaœ?¨¶<(NBÂ?™›™Û÷ç?²0z}2‡?™ªæ/(O4FGL J0912.1-6449?êò\QBE}À&n8§ç:6À:œJNìÀ<=²ôݍ@u±ô¯>ò@‡È
±™?ãHv;?Ê#ðõöç¨@æ;ƒcÍ/@)åËv`"?ï^·E|¿ÃjÓÞcøù¿ãíŸ
⵿ä`³Ô®Bž¿ìª0À',¿ïè,9CîlOTHERglc3FGL J0912.2-6452NGC 2808?â:1?ýŒ?Ä;†.?µ¸'e•=?¯>9Û?Öytµ©?蘒x
?çr¢c|'?È»$^òëë?«<Éb'Ò&?°gïrâ­?ËfDo.Û?ƏÅéØ96?çSÀª^f3?®{Uˆ½·?¸BðÝ/¦Œ? š·Šüïó?Ə"çî"ì?¥¤'žœµA?éxâ×E?ž…néŠoŠ?¸Z«ly©?—Œ"4É}?»ÞΚk%h?"aÚ>?	_4FGL J0921.7-6317?áø䞶ËÀ"Í$žDúÀ:÷I,™»þÀ<¨p˜ïO¯@µÃvâµl@oÿ^ðP`?ÍbvAЯÛ?àÆýòÿf@}ñ'Ž»?ïþޔY#¿ïýSõËÊ?ïÿ¢­>'¿Ø†±_ˆü"¿áÔêp6Ê¿ïÿâÙ~‹÷¿¹à—/'âOTHERlmb2S 0921-630?â1'¸?ȍáÏê‹?ÔAÆeÊâ?Ç?>…fËA?½pã\¨tE?´:ßfù+?ÁL»u¦V?Ä»((?àoˆ¤¦à?ϐjÛ4hÃ?×!ûß?Ìôø(…Þ?Ù>ИŸ"m?´—ÆGÄÆû?ÙI¶({F@?·‹x˜¯Ç?Êîò}Êj£?¤Ê¶énÂ?ÎíùÛ>?ª¦%@·¡W?ã"åÑC­y?³BÐçmZ?Å^zÁ×nÜ?¦>N¸¢ÿw4FGL J0935.3+0901?¸&S%ìΠ@D1'€w‰¤À:&<ì™.À<‰w¦×@	ÌžT@êû܄е?Åˆ¤~Ïê?Ӌ'Û9w@
¸«ôÌ@Ûa:,¢¿èÌ~=šZ¿Ð§ýàk¿ãèÖt¿ëp×£Àd	¿é g´D?Ë¿ïü²ÙÀ3OTHERbin3FGL J0935.2+09034FGL J0935.3+0901?䣚jíè»?Ãúokô€?µ€€†~j?«ATMÅ°?Ñrë
Žð?Â{4aӑ?í‹%`óÏ?®¥Ká9°‹?"HšþËÒ?þ{ÖÕ|?­)ª]!?¤ëª²	Y?å¹+ɂˆ–?±•¡Ý'g8?Áöq\TŸ?§ÉºWܞß?Ç$ß}¡>š?§D+L·Pœ?ëŽ;n±?¢@oÔI?ž÷ó·ãã?…™ìÝ¥?¼X'œ	?¡% 0?u4FGL J0951.7-5328¿ª{ø.[zS?àœ2#iÀ:,F)¯ü²À;€U&£ø@ *úõÿöñ@Ï=ÀTïF?»•«ß}´¿·tA4A•?ùÑ(çÖz@o…'Ñ~b¿ïÿKâCW?ïø›AåR«¿èí][zпÜÅåNë ¿æ—â?$Øý¿ßFôçôOTHERsppSNR G279.0+01.1?âRŽ+¯ë`?Åæ˜t"â†?›P_£ÔZ?›?ÆÍ^-ü?Ù¥ââ¥ëù?Æѧãw@?Öñ|˜W²Õ?Î3bdÆ?'RW´Sà²?œµ²©™¡4?ä=øU×?ÍÕc¿Ç?Û¢›5‰ŸL?±'s‹J'?¨ÈÍ´Ö[?p֓†³Ï?à¢%"Oâô?°ôÊ_	Þ?âÏñv}´?²‰¿eͧ?š
.ë5'?‹ô(kËc ?Ø¿J$LÙB?²³ª4FGL J0955.3-3949?ïGäΩÏ@'ì9yžRÀ93"P>ÝÀ;¦d—YMy@³›­E@óþ?¶=̀{æU?Ñ¥«`@‡…@ñ'©"á@THV±?íêhô¶â¿ÜÞdå1óm¿ä†2Ÿ£‡¿æÆŠÁX¿î¬­½½æ*¿ïÙî§z-OTHERbin2FGL J0955.0-3949CRTS J095527.8-394752?³Š{ÑZ'?­_ܪqN?é÷Ké?Á#•ƒ×?•³;?¹dQ€!;?µ\µ¾š=‹?µÙ`¡®9Û?éªæãVE?Ãâ*F+÷Œ?½S3
KH?¾[Òyÿî?Íz«ý?åi?¯fm/ƒTÒ?â"Oÿ€´$?µT®
àm?Èt½J?ª'¢u"?Ɵ|]NíŽ? Ú±çn?à'·?'Nš?±é 1âê?ӌÓRSì?­z"&´B94FGL J0955.7+6940¿ïò²,LÃ@DH¼ƒ©mLÀ9EMÐÀ<_¶Q`Dä@‡•;;~@[­}|,¡?¨Ù#ƒy?®ø¤
]X@ç*ÙÈ]Ò?ü֘UKáÖ?ïÿ ~æ¿à+RÿTÿ¿á¶Gº©´š¿äß=¾.¿ã©<"?¾¿ç«S€Z®LOTHERsbg3FGL J0955.4+6940M 82?î'+»V›?¤cDp(­?s'ÿI†>Õ?j‡€õ–‡0?­G}[Îr?£²ïY#ý?çƒBiƒ?Ê°kü/C?Äï¬ý´}È?ÆÆl‰ö›?¾‹ñN X?³ïš-5ä?ë2ƒ—d¾—?£ÅjÔe
1?ŸÂÈuÂ? ú@äã?¾{1'iˆ"? –¨Ïü?äùË,	+"?¶múÕ1v½?оÚíOG?µ¨*T
cù?µ6>@iÖ?šC1Î`4FGL J1008.1-5706c?êAhX Å¿ï<Úa
À8¥1G ¨'À:,Þ¨@¿¿>™Ä@>	»j¤º?ľ>ÿðÈ?ÀÀáÜÿIø?ü1¸ðiŠ?ûëøŒR?í'ÜEæ"¿ã°¡óÛ/¿åº &5¿éÜo6ï€V¿ã{ÕctCŸ¿îës`OTHERunk3FGL J1008.6-57061RXS J100718.2-5703358?¡ÿ0@ß_?šà"Ò\Èe?š"Ðr<Œ?¤"</Áo?îfxn
?«ø-ŽÊ²?«ðþeÄT?«ÃûÞ$?¨§iEÞ'E?¬ib©¾?ìÄZ[»ÁF?³+êPsV?¹¤œ¢ólö?œ_eȽ?·–Âîõ?£7^q–Ã6?éؔ
ÂðÏ?¨¯˜æA?Ž7
"ócº?x2)›ÄÓx?©9ƒìr‰Œ?"†à"í?íó‹Šå	Ù?"ÝYW£4FGL J1011.1-4420?Ê7£^®%@#b'è},|À;2*߈'À<‰3úÙO'@ "«#Ú¦?ÿdž!Ðý?Î['ãG¯?¥ñïñêém?Ý'½†,@¯»ù9¿â˜éÛÑLŽ¿ìez]"/Í¿à¶@º°@¿áñ–`)5ƒ¿š¢ža:¾©¿æÜ¿· ìOTHERunk1RXS J101130.7-442241?è–ù3Vۗ?À'³ø ͯ?e¹N†ßE!?YÛ("SU?ÍM5ø‰?Àª«+ê?äwê°
K?ÌÃßzbË;?mfé‹ïé‡?×îñnH?ÖÕ^ˆ—?̒-RrnÆ?ê-²X"Ü?¤µÛîkÞ?…Ð@C1	£?peBÞJñ?Åì3ÞjÛò?£Àv){(?î"öÔËá7?')½1?LÂN‡¸ö?Fs¬Ô)v?­`‹ªÍ¢?'1,f£4FGL J1018.9-5856¿¤¶\"‰²¿úõ<WŸ#FÀ6*OÁß3À9­HJ­@øhÑz±w@rÇZˆ?•0£¥XŒ?Î_
¼òd6@6]3]$žE@/È´²¿ÊŸiKs¿àm	]¡Æº¿åyöÁgéÉ¿èàÓ¿Û¿í#>=ÓJ?¿ènq—òÐmOTHERHMB3FGL J1018.9-58561FGL J1018.6-5856?wÀ‰''/?}ŒI•?èK;È-?ÏL"œ|û›?ÎðÎÄÎ5?Îï'þ¾8?iÂüxeÿS?x™#"Ì9¿?íÄ¢£qQN?³ˆ,±'I¦?±Ó²EŒ?³;Æ/Wxƒ?®ktY›«?œ(¼hYZø?ßl 
ޜ?·(jÛ6/?ÜƃT¾mï?¶"ISÚ7°>¤&ŒÝ†	»>­I×»5
$?íîáa?¥)­
ò¹?°Žþäv‰?¥)¥çÃú4FGL J1023.3-5747e?ºÐjê_Ê¿ÚDUšfH3À7×xFÜ]À9›mjW@#_Jé2^@v¹<Íé?¶éπËf¿j&¶Ý?¾50¼ê¾@"Ǥſí(@éÈ?ïY¯¾ôòÜ¿ë[¨«¿ânŸð˯–¿ã»>U¦¿ÛþĖe×OTHERSFR3FGL J1023.1-5745Westerlund 2?€û™'¤2?†	0±Ú"?G‡\Uüâ¬?Rµbªû?ï¶/Âßð?‡ˆ|y(é?¤Ìþƒ_"?°Ü8:oÓ½?¢ïÌÜ?±lõˆ]2t?í">êüOv?¸vþ-\s!?¸[Káz?Ÿ¸_ëóN?®Îñü—;[?–¯z¤7ZP?맀p?£
%ž*í?'·Ó;Ýð?t?·Yùo©?'bü¯:ü?…wÛ·v%?ï*«µ–°?ˆ;

94FGL J1023.7+0038?{Z1ÀQ@Fä'úòÀ8Dœ¤æÔ¶À;ýÖ.u@ÿªó3=ð@Üb¼ºh?¡žÞÁ°¨Ä?Ç.95×@"2¹o!öË@½€šFM?·Y /_éõ¿ßa}H€!¿æ†_€>:¿èÅB>éË¿ì3ŒŸ`-¿ã'?´‰	OTHERLMB2FGL J1023.6+0040PSR J1023+0038?íÌ®Éýރ?«ŠÉo'`¯?­-Ñ{ÐÊ?ª*ù²{?ˆ"}?'Z±3Ô?ï^Íì[y?"('¹þ†š?c¡%:ŠÖ9?q¬t–?'²7[#67?'˜¨ Ô¡?íAðvˆÿ?¤*'M±m-?°gÙÓ&?¡Ö–À	3?Ÿ3\QǓ?_×8î;Ó?ïÕ6#Ì?fã3¬uÄ;?_–:xçŸÄ?UÒg©(TÔ?k2¬ŸÀ)^?`Õâ8y£g4FGL J1024.5-5329?è¸j÷^Š"@
çDñ¢À;1#³co;À<']9—@"?Öê‡ô?÷‡åÂg=?Ö=…³:?ÞAãd¾Æz@	0)®O3D@™zu<¿ïÿþøþ"¿Ê0™Ã?ïÿTßUe¿Á¡;#—Š¿ÒUÖ¿á±÷(ÀéjOTHERunk1RXS J102441.6-533141?뚪˼?¸Q›óäæÉ?uÁ¶çÈ?Œ%ýY³?¿A2ˆÐÅ,?¶ˆÕð)Ø?ã¹W»})M?ËUÎےÀV?‹pçÞáâ?£Q0&€?×±ÉPF¶V?ÊMÐ7æÞ?éÆn¯uX?¦¯W{0[&?¡~ÛK^r¯?^úÐ)'?ƎoSâ?£½LN–øj?뺵
T?¦*"ÿµ£?u÷`H3S¬?oÀ¢K²·?ÀepÉ{ð?¦QÛæ?4FGL J1024.5-4543?ÄÃ|äN–@#Àd©ÍÄÀ:´úŽ¦÷À<qZ»7y@ êÈÓmû±?þ"ä0—?Ä0³|Õ9?ªZÝ#å•ú?èaþÂé<@_£Ùäbk?ïéè »6w¿àN¦@Æç€Ç¯;¿Ô]´;0'ª¿Ñ¢5Ÿt$¿ãµ\"•¬$OTHERunk3FGL J1024.4-45451RXS J102430.1-454401?æVððPYX?ÃF¼ŠPJ-?iՃÎÔ?jû¥@£k?Ó tW±A?ÃL8ïÎhŽ?ߨrkRÂ?ÇÇR‹»Ã?zP\îå?‡kÎñ넇?ßíL¤ ñª?Ǎ¬{Z‹–?éÚLÒ}	?¦|{l‰è?…¨¤g˯?m"‰éÜY{?Ç<C'9[À?¥²Ÿvëà?ë͓{Äs4?›±AüP?†á;!gŽÒ?wž¯…ªd?¾·<½¯t?›j6µ´–©4FGL J1029.3-6657?éÈå'tÀFr*rÀ:…úcÞ̪À;ñ讪¢Ö@ŽöÑX!Õ@WWÂHå?Æn=à¶8·?šOãÃ?Ø-™–>›F@Ï#¾Ì?ï
–V:‰¿è¸…íë*†¿êŽ
>¬ãù¿Ý¬ºÞ¿¿ã›â´•žb¿åPT "žXOTHERunkPMN J1029-6656?홸ì^Mj?ªŽÐ6øÓ?b5Kº¬¨?ZºJÁ¾‰?² Ž?8/o?©ÁØÄ\'?éœ>
±¿›?ê'$?Bº}zIÕ?S`~c$?É|MK¾üH?Ã:b¼Ó?ë­¹NRÒæ?¢ÿæ;ã"•?…ó…OflÉ?t-¹"[ž?¿ÓÄã|›??¡•LžàÛÌ?îoșXDé?ŠV­ïWA?`}qAA@\?LBdp&—þ?§ûŸVgl?‰êPgx*4FGL J1034.7-4645¿î3U—k±@#Û,B»fÀ:ïùZÊPòÀ<cÐÜ&$@"pçɨ@'}ô!¥?˵Ï_‹+? ¿5#g'?Ԇ$¼øÄL@¹9õš }¿¿'£ê¿ê±(+˜4¿Î§!—¿æ]gÿî<¿ÊçFu°0_¿æÎbß\\OTHERunk1RXS J103438.7-464412?äõ_"ýF4?Å('ÂôJ ?b•}æEÔÇ?YÖ÷Ÿk-&?Õðú8çð?Å)àêZhÛ?ëP=™û7¬?Áa"…χ?g,"bxj©?z…ÏPÿ|é?ÂbWF‰?§?Áˆ‰ˆª.?ê%#P_¦?¦˜:Þ?‰,ÕRßr?tÜ!r'i?Æ0žŠG?¤ÏV+Ú?îEôá¿w?‹ÌÆR<ü?O¾3±+Tý?FzÖ×P?«!¹![+?‹¾úç•é@4FGL J1045.1-5940?"߲úàÿ¿ãüpÿFœÀ6høj	‰À9êƍîj¬@î«Ä¿b@©²=ÕM¥?'Šg!¢<*?¼Ø;•ØCù@'Ú^±¬@¿+½óëö?ï(Åñç9¿×q10–v¿ãì2žðÔ¿äTµÏZEÇ¿è°&äpX¿ä¹Ùk€,OTHERBIN3FGL J1045.1-5941Eta Carinae?ÎïW,9ê?Ç5žU´ì¹?£œ¿öÝ?­ÐÁc­g©?ç
jò‹?ÇÁäÅÿ"?°Œ]X£Ð%?ÂsË»à8À?á0ïuC>?ÔFÞO«¾1?Ù¸†Êì…z?ё.´É»?Õ.pkCÄ?¶¢:‰¯¸f?·r}êVW?¤ŠŸêS3d?âzx
Rý?¸Ù\ѳ?s¥ÊÈÙº(?bžÐ"‹·'?ÜU§wà>?¹nN­>¥?á­à®~-'?¹MžÃ'A(4FGL J1045.7-6414?çIiÞôuÀ'C{À9Ϻ˜í¢/À;¼áG®{@báK´ß@"õ?²w?Ã>ZÕÈI?Æl–\ò@\,CTéf@裉1—}¿ïþ¢˜›Ã?ïúiˆYÖ5¿ã÷M©Öþ¿áJ·~†îœ¿ìSá~Š ¿èú˾!OTHERunk3FGL J1045.3-64141RXS J104537.2-641438?ê×þjÚ|x?´%Öy`?£¬~¢-Ú?dӐ‹?¿iÍX"…J?²'ÿ N™ø?çô&ñÊ?Å;¡?lP?{×°IêÕ?‡P÷?'Q­?ÑZ¸ñ§œÁ?Äð$œù?æåЂnü?°\\µÁ¹m?­]s¦°&s?•¶€çŽÔÝ?Ía›òp?¬w²þT?ékaV¥? Ãe÷¾œ?®&³RÝ?" úM
?Äd²Óv?V|ð¤ö4FGL J1051.6+3253¿Á9íü66@OÃ˼+"ÙÀ;'?Ï"èÀ<êՌŽï@û´ò»sß?ÿ†YJôðØ?×ǘšëÿ?©	%B¯¨?ѱÁ"õxh@BÜÔ+æ¹?ãxo'Á¿ïÿôw5Áƒ?ïýއà3²¿×E;ÿ	µá¿Ô—Ø"¿ïÿe`õäOTHERsbgNGC 3424?ïÍ=Èýg=?ƒk3Øÿ?,ÙÝ´c8´?/Rº¡±ë?xzL"©FÙ?ƒDéê¿~?ïǒO[,¯?‹(kãLâ?/àÈåËx?EâjΘ?{7Ò@º·?Š`ˌVJ?î<°+'?–XˆT÷ty?a²"Jbv?`F7ÝÖ:?«,DrØ ¹?•ÙûÌ;?ïêÝEª?Wåûhá3ü?f#VwJ´?þÌCèNn?evŠV`xÅ?W¾¾`6&Š4FGL J1059.5-6021?ì#%Êûøp¿Ü¾Ò
SÀ9³9ä'À:š>—ëC°@lTi¹­
@ªÂT£Æ?ÊäÑ{]C}?Ï$_ZÙjj@>ä\5Šü@2\sž]?ɖƕüA?$Ç/¿âa4x­'¿æ¥'ßæÚë¿ïÿýç!é?ïÿ·pD5ºOTHERsppSNR G289.7-00.3?Òª-Ò·v?Á
)³aU?Äߝd¨?¹%®ÆÙC?ᩱ/Kê?Ãà+ô¦Öü?¾;IOÿK?º®>$´?°"gñF?³¸‡ Â	?ê(Ø´T?À""á!$?ÃQh0¢Zå?¢À£K­?ÅÌî€&H9?¥ÅʄX^í?å¸jSÍ×8?ª&Á!?¸­à1|G? $ÂÊ?´¾w''‹X?¢F–S—û?êR?©§_³bõÅ4FGL J1114.2+0638?Öiªþñ¸@M'ËÿGs\À;¾vÌ7«À<Ø'QT†@"_©mø,?ÄWoRž2†?åÄáçDò?ïûo! ä'?þ8¸É	É­?ø2¥4M¿éç÷Ë~4¿ïÿߞ¶Žó?ïÿ.´Hq‰¿äÑq5Í?ʌ3)£'¿ìYƒ)Ì@OTHERgalIC 678?îÍlÉ°/—?¤¢5Y?zjæs®7 ?€N—žÑ†"?Ÿ·­-h?¢/¨Mž?î8óÁËÍ?°x
'?‰mFb#4?Ÿ¤hêûa?¦}K`zi?¨ dhxµ?ëî+ÙÃê'?¡õ"@ÂA'?"´ì>Œ?¢»`FG?¹'@¥›Ô?@\N.ï?è<0z¬Ð?Á¦KßÏð]?>7Ùå?Q9´\9BO?Îÿù*ŠFQ?Á©Œ®0¹—4FGL J1128.2+5831¿éè›
`Î@K¶-VÀ;b°+¬VÀ<ёúhçJ@Ó£åLöS@îÛŽ,?Ð{uâZR²?¼oa^®?íÝe k/y@Öm¹kñì¿ãPxˆ§ÙοévýÃÝé¿ßäY±L¿âmf4è?¿ëўJÙB?Í×͜U‹£OTHERsbgArp 299?ý5T?šOogÍ!r?k"Úó:?_/•÷¿ð'?¥;R‹
˒?™Å¬½M†[?îñkÕv|?œð'øÛã?c¾|/ ÕÜ?mc`ú^Z?ŸZµËLdé?›S~`Ñù_?íÐÚ×f%|?"/DÄýþ?ˆ(NäíÍ?~b³–b|O?¬èNõälÐ?ŽûOwù#?îª#ð?câçW?q­†!ÉM?c\FŒÑí?£(®I®×å?ƒ
ZjÐl4FGL J1151.4-6248?劸'ñ~¿çz¾ï>'À9!JÕh-À:À´†"éß@'éçÆ²@ê²ái<?ÂøScTc/?±¨Ã
†P?õ§ðª!§@²™Å¹?Õ-GáÀú²¿ßø€‹*Á¿ê¾9÷r'Å¿ä"ô¿7G¿æV‰äð°¿ëaÚ`3F~OTHERsppSNR G296.1-00.5?¾Ó‹-7ƒ1?±²B#º®S?£µ«Œˆ""?žMW$%1?êê3ᐆa?¶*±jZO"?¾°€JøÅ?²£•Rz§ã?'–­BÄ2?–«DÀŠZ<?ë•:Œ¥ÿX?³û7…O¶?DZ.‹¼H?¤ïŒ6 /U?´dëµ1ß&?—yÆ&P]?ç«v=¶Õ	?§1><Ͻ?Â&à³`[? }Õδ^Ê?§54¿vòÍ?ÞÀÙv?êô‡0z
?£Oî6b[4FGL J1152.6-6207?å÷u #È¿›N(¾ rÍÀ9ÕrQV3éÀ;€ö4¥#@åQ(À@%iF·G?Ô: $x/g?ä{àK.Ò@Rµ¼åÎü@Á'kՑ¿é%÷@=ݱ?®T˜€uv¿æbÀi'¿ë›[Õì¿êC,oʓ7¿ïÿü¥¬¨OTHERsppSNR G296.1-00.5	?·ü]؊Â?®È¡'÷—?Ãå'üØÛ¡?ºÆqš³]?è*E¸‰?À=Ýz€ð?²vZ?ζ¡?°¥³¥Žè?·¡òçw?¶ªGcmÀ?ê¼ö[#ZI?¼Ãuö<»S?Â-\'_œõ?žÍ¿æ*?Åô¯°rr?¦"'¨þð?å÷}
'<&?ªàUÖBðQ?±µšFɚ?"Ds
7?ÆäÂҐ}?©&˜vÃ?èE†rê¯?«¾'9q¤4FGL J1155.2-6259?ÑçÅb0‡î¿éè:ÛÀ9'6TOãmÀ:—yóáäŒ@"éµæ¬G@¸5u-?òƤ^ïy ¿îL?á&£7¨ú@Öð<=ž?ß¾Y¢2ÅO?âKÕážk¿ç˜}Ú÷1û¿æ/Y‰ß¿é«^½ûx²¿æÓ¾ŽE¨OTHERsppSNR G296.7-00.9?ž2\Ô¥;?·Ó6
"šW?©µŽÑL¢?¶ÝTÇ4?ís2f?À
yòÞÒÅ?¯¦˜­"Ú?·=·Þм?"  š¥ëÄ?«œ¯éÿ¥´?íd•pQŽ¤?º  áÝ>ë?†&z´?¡|4?¶È‹½|"3?Ÿã†Ù"ÎÊ?è…dé£zš?¥ª£àÔ"?¿"nÆkÌ?¸Õj˜×íQ?r]a!óÚ?…üe{wôp?ëè·dü Ÿ?¹Á¼4FGL J1155.6-6245c?т88º¿â'óøŠÀ¹À9+û¤P¬ÁÀ:lE(þüË@Ö*%mwÓ@íÍÛÀ…—?ËJY™??Ñäg¾U:Å@‰óžÈ­ƒ?ö'ÞÉN"¿ç€E4½vî?熁žü?ŠºDΪâ0¿èÒ­N ¿ëfÖ-¿ïÿõEq#OTHERsppSNR G296.8-00.39? 3Å̇Cé?¾KEãaú?´+{W¥œ?·ùàÇ×(Œ?ìwT8Bén?»‰GZFäÚ?£kÍåXl?¤£ün1?ÁuwÂß?¾sî¥äÌ?ê'~'Ó¹Á?½Ü âjù
?¸f»NöfC?"Ue&ܔe?ÅA|·¡N§?£eñ%Nb4?ç¢Éh8ߎ?¤"Nº^ί?ŠsB›ðùþ?vÜ&nÚÕE?Ç&†'_n?·ü`*م?é̑kÍd<?¸QPLú»¦4FGL J1158.3-6232?Ÿ±'gSÔÇ¿ÒØ>e@v"À9)Þ®v pÀ:½¨ö-ï'@ XQÀ'ô@Jh˜q?Çm™I'›?Äug5CXÅ@nÜV­Œ@»{–¤G?î"ßÄK¿å´—1š­¿æÂB/Oy¿çñ§w¨®¿ë­ÌŸJ¿éë֙Õ)OTHERsppSNR G296.8-00.3?ÐJþ™™Šö?À¹Î.¢ýT?¹Éé'9?´-lŠs5?ä¡CP
=?ÃËoXåä?®ð|Ëx?«ó¡vd?™|^¸ô?œ…ÎBëÝÕ?íV_Õ=?°´Ï`·¤?ÝÅÒQ£?³ýÀŽ^©±?°Þ‡GC[1?™'@eƜ­?ÞO[ޏ?³†uóh;?´9<z}*U?šj1>ÿvÈ?¯÷Ì»äŒ?¡ªÕ1¢)?ëy[°4œl?§U,à94FGL J1159.3-6122?ÂGÉ|O½?ëýH•›À9Öƒ.ô	À;šCㄟ@Jö‰‰¬@¼*`%څ?Ì)ž‰îUß?ÉŌ§Ük@_î¥d¨÷@dHÔÛ.?æüóÁ-\Z¿Ø¶ßz¤`ó¿á-ÆwH5ú¿æQ6É>£¿î	¡Ñv¿ïþÙú²¹%OTHERunk1RXS J115843.7-611934?Ãxõ"ë?¶šÍlÔ<Ú?²©`§ZG?¬öÖ+HÁJ?èÌÒí¯³d?½\†Êô	?Â
Ã=´s?»=v¬µ? r"ÒÊ­·?£wi&Íóã?êv&ãf8]?½%ÒEqÕ?Ôf¶²'™?¯2"^œHy?» mþ.×Ø?37/éŒâ?âh—4àÜ:?­DN‹3dW?Ë™ÚSMÛ?£tÔۖ?ð?°û¿lÑ5?•·&P嬐?ç¡—]'b?¥;êÁ÷õ4FGL J1208.1-5149?åog¼|È~@$ô‡Tów\À;t2À<kAHŸ¬@ oÔn+ן@.Ʊ?Êœ§@ W?¬éᅖ'c?äõ"FK=ì@9ʎÙø?ïÿ¢­>'¿é̱‰zg¥¿à˜Øÿ`ö¿ÚJS`OK¿éÃsݝT?ÌtÀÇ/ÿÍOTHERsppSNR G295.5+09.7?í´¡Jȶ?¯M²°?kª~'ïŠ?~‰j~§ó£?±}¥5Æ7è?®¿;AFµ?板@?È&‹Äõ©O?o«Cñßès?{7+ƒœ¯}?҆uùÝÀ?ÇþXObu?ìmd}2©?žð³û#¹¥?'*'ò/?tZÃDln‰?ºO›
NÍ?bÈ/0ÿT?íiûŒé›?"›nœ%ÑÏ?u:âŠH¾?d¯ž÷šª?³\upBí?"‡³€j¬÷4FGL J1208.5-5243e?ßyðŸS²@#0FÜ]dÀ9#V›‡À;ŸâV¡ÍE@ eSµø ?þÙû‰xº?«¬=
LŠ?"XÖʖU†?Üyb—yÚ?øˆmÅ*l?ïõ΃†1Þ?ïŠIˆà¿á÷=^ZS^¿Ö&Å#
F¿àêâ«¿ØÙ	Üwº¢OTHERSNR3FGL J1209.1-5224SNR G296.5+10.0?ç‡LFÄÍÞ?À‰9W—Ÿ]?w
WH2»'?q^°â?Е2U™U?ÀuÚä«îº?å#:ü9?ÌÕ~σ
§?–Å¶"">?¤$½V¯â?ÔOó.žªK?Ë¥]Ç
Ã?äîTŒ¥¨¡?¯#n†íþ?žñÿsl?‡Šl‡úõ4?Ô46î¢Ç†?®!Ü¡Ê`?ä'u镻*?²Šc(8¾u?Á,TQMŽ?©#ý[?ÌÉÔ ÅÉ?¬kÈG9C=4FGL J1213.3-6240e¿ï¹@󇙿À=çՒïÀ7@)íÀ:,…dž@™bRZ•Î@¨]Ywj›?¡‹:ÜúA?µXè_¶…@lâ¬2#@z$b_ñ'¿Å¥'Abv¿ÕàQ<¿ãyâyÝ;°¿äv†¤ÊOD¿ç#ĀM`¿ãhë¡y6ùOTHERsnr3FGL J1214.0-6236SNR G298.6-00.0?'Õ{Ç?ŠÅ(†Zg?¤Ï®$çð?©éñŒC?î"Æu…¢Å?­æ<Íð??JÂN*³\?"'µ–ív?ÖZM;Ñ{u?ÍÞ6‡™B?äU®Xޗy?͵I«	õ?µ—Ôï'?Ÿ['†ÿf?»'$.ü8?¡Q
P։?éï,À÷¢‰?§ø§ôâ?‡ ºì…?t•UÁî?Ëám«`?¬;/ÃW¢?è©!«î?¬}‹Ì䄨4FGL J1256.1-5652¿Ù‰hôá@ùú}	@À9Ð)é•öÀ;¤uÓÁ³"@/=;tË.@"|tÅ¥?Æ-+²5qÒ?àD@÷–û@{xÎø?ø=ìl¥DÉ?ïúÂT£Æ¿Ú%›eK´3¿é1¦€²Âà¿ëxöLÖó¿åŠºÙ…Aô¿ïèP¶Ñ¸ÅOTHERunk3FGL J1256.1-57031RXS J125554.2-564945?Ä@ÍDÔè¹?¸{ºIÆ?·"éõ‹û%?´Ÿ}¬t?èopFm?À›lG'š?¼g¨ö'Ò5?¶Hÿ»Ås½?×Z7žFR?ÇãÝ9´ó?àÆÅ^¢'?Ŏ-_moT?Öôcðß?ª"7°œN?ɐ¦}^·?©2"
—´?ÜCHÑ$8Æ?­˜5³ö/µ?¼¡Ä¢À2ó?™ï¸2%?ÛçÎûÉ??¸îÒÁŽ®?ÜïÀ¹T*?¶Ðmç²ÓË4FGL J1302.9-6349¿ëzð5¹©¿ï"ÃÀ8Ôðý-½¨À:Rj¢Ž5@;ó HŸ×@#v"Á›@?µåš¡+‰¿µý 1
i@\[›1IN@î1·?ïÜ<a/Dç¿êUÈßWhó¿íÉÂVQEm¿àÚ!2Æ¿ædÆ®0*?¸iE~d^úOTHERHMBPSR B1259-63?äé·¨ÈÍ?ËWH՟mO?o×¼Mõ?€6-ê…?Õî…'>í/?ËVá( §m?ì -úPâ?Ã>JåÒz?G•GÂLt?eº0r™ž?ºÏü¨ßþ?Ã5º/k.8?äzzcs¸?±â[Uï8? üÒg	…£?"+ë3ÅÁ?Ôëpì8±Ý?±vf^ ½?ê,m°¾ã~?¶é«{Ãv&?@8ÒPLª?7ÌÿÅ»¸o?Ç>jù!·?¶ç'1Ǎc4FGL J1303.0-6312e¿ìD>H¿ÖáU…m'«À8EñÓò[À:ҕˆ'á@"'|2iµ?ýÚ8
2ˆé?ªO"›Ø¿£e">=¨W?÷ˆ•âU?ûÈúDÕ'?ïh«…Th7¿Ø6rûé¿àÛ?÷fÔJ¿â…`\a)ç¿Üíaw¤Q¿ÃQu¾sÐOTHERPWN3FGL J1303.0-6312eHESS J1303-631?²V~ôÚ°l?«£'X–à®?wŽ(´x—©?tÝÈl?í†Ïû¸Â?¬d"@ôƒc?Úa‹™ˆ?¨Rdÿ|?˜Ä¤£&ñ?¡òEÔþ?îKΎK©?¯O-súE<?Á‹2ÖÒ?¥éÎòˆ?ªàÜt=? n@cæª?ê
[']C?§ÒExÕ¿?¥³ð_Íh?'fBÆ{S¬?³ò"
Â9p?§?ßý˜'?ì&|¸ªâP?«ÙZ÷v4FGL J1305.4-4928¿ë€~ˆ ~@*«h'0ÆqÀ96s¾=½ÑÀ;üR$A@Ò@VÝ1t@êù>?­7›!Ùïu?«ì^Ó¶²?üuÞß)@¥^¿þÞ?¹j£Œâ|¿Ø¾U{1¤"¿å™ç'Z¸³¿á¾'¼ÞB@¿çpÖAj®u¿àâ~å¹-OTHERsbg3FGL J1305.4-4926NGC 4945?éIHj-Œ ?¶G²wÐÜÁ?–!I›cÐ!?Žþà"•?ȵ#ÝU|?µ‡Àø	mÝ?ìÚ92ë;?¶ì9³|/E?žÕ-5®_?«ÿ$dŒŠ?±xî3: ?¯È<—H	Æ?êZsÝØ?§¿¯
_t?¢K€€&D?Ž#ԃ•†«?Ãb#¶?¤çŸi÷›r?êd&•uË?¤Š¾'8?³V߶oñæ?–»'š.U4?¹‰ä_Â?š3'íª4FGL J1305.5-6241¿ïz=]P	¥?Á9Û×À7Ù\M}À:\Ê4lW@xƒ
¼L@ãö<1ßv?­R°Å/J?¤§Q"¤q?öéëÜ\ŒÉ?ùÒ¼­ð¾š¿Øž½ûx±Ã¿Ú)²ÒÛ¿âþtàÀ˿㕮Þ]¿è¨Ÿ%ʔä¿áýiíÚcŽOTHERsnr3FGL J1305.7-6241Kes 17?¤*ƒb¦1?›qøáÏcÆ?ª
o]ù{ë?«ˆžÝEª‹?íÖaê=à?±?a•qx_?¤§uü?«0Õpݖ"?º¿/Ÿ°?x?¿u†gÛº?ëg¨¡™à²?Á¼æÁL=?º§^ÑëyÃ?žÁ'œºŽ	?¹`%D'g?¡¢úÐû·â?é}0M{?§9ßđ~?¨Xé‡Yi?•ñá{:ó?¼g¥={z7?£¨Ì¿-°?êí|¿ÚÿÃ?§{I1ž¯c4FGL J1326.6-4729?×?««Y@-êy5v'À9C	A}À;å±^²<ÿ@Û¶ˆÜÌ@KÌå €©?´"=l@?àùíÌ÷"÷@'eØם
g@PôF¹?ïdC¬':׿ÔPá_ø¿Ô¦êk²¿äè+Íä¿î¯4¬¿ïÿÿ" 5•OTHERglc3FGL J1326.7-4727Omega Cen?^̙a ©u?Vxè21?ïÙÌ2–·?kpCÎÅ8?f̀¸x©¢?dÕ×1\z§?uÂ[ÔPÉì?zιÜDÚc?îëácÑcb?£¶RÞ,?<¿a9?¡ÖÍwIäB?'4†ˆ{D?€çnžvô
?íXƒA»ÐP?"[­Z_Š?°µÐ^©?òÜt"?W˜¸Ü?E;þ6?î)€Ób?'ø®W"aÏ?¬¯Æÿ²?'Ì(¹4T4FGL J1331.0+3032?ï¡5DZx@T+ü27‹À:ւè},|À<›µäRûP@ž&ÂaŽæ@ŸŒÝÉtS?Ç`ñ\y'´?ÅüÚ܄ü?ýšMÀg?ü´P^è×?æ)ÖÈÏK¿çñ¢ÚŠûq¿ç`Á`ÝæP¿ÚOó]ZN¿ì°-…C¡¿ïýM"ŽÇOTHERcss3FGL J1330.5+30233C 286?îøÌe3Ã)?"ì(Uí*?4ª ò¾?†å_˜à¨?'L	Ù?‹dÖµ—%?íßëlIT?°Ø/çª?›âWV‰ì?¥*æy¿@?¤ZúS?¤Gâ".3n?í†úÆQŸ‹?—!DB·x?'<N¨'?'¿ˆzÕ9?®rHs'Æ@?'+\ £C?èBh'¡â?­ w_c?ÄØù¿9?¬Æºí£Ìâ?µÛù=4¾€?™!¸ÍÑŠ4FGL J1343.8-6208?Ú߂íП?»õ|"š7À8ƒ%{º‹'À:E×z¥¹@[#¨üŽ@ö"|#g
?ÆGX™Ÿ"ð?½|_LØ@-wœïo?î~՟ž?î|äù¿ÒŒewS¿æBaP™¿çÉâ!GÎK¿ê	ÿ\–¿åì†;OTHERsppSNR G308.8-00.1?¨ˆƒÿ_ÜÛ?½í[µ‰
?®ãAÙÜ‹?µØÀt¹?ì‰C¢l@ú?Âô°2…Õš?"â"§Á?œ0*Ú]?¶¸ô÷›Õ&?·Ü5£J¬?ìÍ@‡GR?¸:ÎÌ}³8?³.÷s¹pÅ?"³øØãðÖ?ÀÚ&®±J%?§?,20=Ï?éc—eÜ^?©]^/
<+?r:ïiqÿý?`¸"D¤È‡?¶˜50¬¨?›Ñ'-¡×ú?íƒ{™L?œ"%ðÓ¤Ç4FGL J1344.9-6228?×P~Vêj¿ÏnëE2åÀ8¹ŸœÞÀ:4܃ùõ$@è8<ÝV@‰ÔDRÉ?Å¢ÁvŽö?Ý[ÔýrÜì@ìý
y@,:Z™Ô?ãH¶‡æ鯿ٕ˜ƒ$"¿ÚMy£¨¼¿èˆôe˜
M¿î¦âÂØWE¿ï×ÁÝÛgðOTHERspp3FGL J1345.1-6224SNR G308.8-00.1?ZŠh!ž1»?P£ˆ€±)?ÖÞÞ"bÉ1?Çp»\k&'?äƒKº½ÌO?Çu¶v²Š?•¯Ã".§¦? aÛª‡69?Ç7úÐg?À¢yŽ:å?鄃/cpþ?À'¯þYã–?Ÿ»cqjh?"r]%'?áwö,œî?·Yr?ÚãYܖ?}?¶-ÿæn¤
?d€ÕOÎ
«?UBàÜÛ/Ã?™ºrMj;?ªæ)|5Ú?ëEŽ×c?«+bÐöœ4FGL J1345.3-6253?Ú›4ƨ"¿äâÙÿePgÀ9L[[piÀ:¼2JÕç@^WÏâ@ª*sq?Ïý‰˜š–?Úò²Ú³?]@!móùa€@óI€Òx]¿ïñ7æ Zé?ï•dSN\¿á`ÊžUì¿ç{wÀ*ýÛ¿ïÿÿÊPË?ïÿК·¦ËOTHERsppSNR G309.2-00.6?Ñó€Lbō?Ԗg–~‰?ÃC>æ¦N^?ÁK«Õ)•?â5p %	¡?Ò6PÑ.?¼½ø‡?¿aãõÓ?¿p«¨ØÐj?½'åà<¯?èzHäÕ?ÅÁVï?À}Vžåˆ?¡ë˜*=D	?È÷gŽÙ?§õÐΈPr?å¢Ðtö[?ª"ÿ"'«?«§IõEÓ?œÞ@ír‹?²°–?óë?¤}#z®Î?ëã¤Q?®BKcŒÊ4FGL J1355.2-6420e¿Ô(é°T¾kÀ•;›·À9¶N¼üuÀ;w™÷j·@%tÁ¾¢h?öªî «†?¼wbâù4	?§¥C_¿òã?êyÔ½\@UaµQ°ø¿ïòl~®[È¿ïì "ÚÅ´?é•\¾Fø?ïýaw]¿ÙÆ|¼A%¿À]GóÐGOTHERPWN3FGL J1356.6-6428HESS J1356-645?àÑyFO?ÍâÑ_–ê™?uL+'‹úï?˜¯^8÷ð§?ߛ,a9Cw?ÍáÇ´ŠÇ?Ý>çyÄzš?ÑùÀÀE?vXn®ú?"R²%X5ò?á4\låV?Ñ×JÅDž6?Ú30síã?µ‡iùé'È?£28ð¹Žs?Y"q?á³D7gð'?µ†™øNo?à6E(»?ÄEŠ!Y#´?Ÿ€x5äL?•QгJ?Þ¥ådzÿh?Äq8y$"Ê4FGL J1357.3+3730?•ü}ÉÂFÛ@R+µ^ñýßÀ;ÂD—Å¡À=ÅÉ£L¡@ k°'­¼ç?û'²z;/?ݲ~ñ"?ÔP`j£âÉ?ö‰ì˜D/?ú(¥é34á?åŊƒ| ã¿í]ï3ÿáÍ¿È`—D€¿áY+€Á¿Ôãr@9V
¿ïþëbº	|OTHERgalNGC 5380?ïs4=o?ž¢%÷¨?rÇ"Å.Ö¿?uƒ:èã%£?š_ÐÎLœž?œ[Ÿ-í?î\àéé©?¨z˜ÞGc?ƒ\ÙvñV?'±/)q ?¥Zê«	'?¥+ÉÒ?ì·3{÷@?¡êÁ
ÚÓ?"s|"¸?"ö0Bêät?µ)Ÿ&/ü?ŸMaè+Ó?ë}Z?·ì?¥´—bƒ?ƒo¯ø.?¬Ú$œ?/?ÀÙ|¾ Ë?¥&'…Áˆ4FGL J1358.2-6210¿í¾ùKA--¿ÓwÂäì~CÀ8SÒkr>âÀ:WoÈ@ã'4pJ@[#<E*¬?»5€•f¯?Ѭ‰á?Ër@íwàmò?û'ºz9×è?êœâß]É	¿ÛÖqüœž1¿ãŸÕÞCl¼¿è±·Ÿ¿ì踻Ð`¿ïýáÃÔ×OTHERsppSNR G310.6-00.3?'pæ·\?­üݒG±°?Ó Kft3ž?Æ3/)ÄfÀ?å߮ŏÐu?ÆÖ14{˜Ø?íù~S?3àŒ)ð?Õɝ±?ºŠ'"A'?ê£	º§ $?º =E¹žô?¨}&]œZÈ?Ã5Î`?Úh©Þ>Rñ?µöŠ	O®Ì?áCØ«Û?µK"É"ÛB?]a箟·O?N@&ì·{?ÂÚ`¡§î?©ðãl£÷V?ë@htF)?ªfÁÓ5ê4FGL J1404.4-6159¿í·jŒ)³G¿Ôq1Ûð+LÀ8!‹P*º¿À9µ+†–‡–@–#BzN@í§m—³?Ä9å>ˆ¦Ø?Ø+G¬fû¸@…ÂL@J?ÿBe"C¡À¿à-Ný¿?¸óºLl•*¿åA1ÃÇj¿ì4œŠâ¿ï«±äéú¿ïäa¾áҘOTHERsppSNR G311.5-00.3?"[.—?°·õ³=Ra?Æc*:.?ÄþL½Mŕ?éÜ_ÅÀµ|?ÆØÕGZÞ?ŽÚٔ³á?'³Ðe‰?ÏõRN?…?Æ؀)í.?çŠ@	ç?ÅÖaxþþ¥?¬B5™+?–G$‹¬q?ÐÏ)ôô?³‰]í72o?æ6YHYëô?´'ùx,ÜS?N¶¼L¯ù?<¨6w?Å_láÜù?«â|ÖKü?ꠁYÙ®Œ?«èß«‡4FGL J1406.6-6523¿íúŸpž"ÀÀ
IJFu/WÀ:;Öç‡À;‰5
þÆD@؆V›Ã@,ò;ò–?Ǿw‰ú?L? ƒy`'æi?܉±¤Ó3™@7~'«cœ¿ë; !³ƒû?̤ç«ud0¿é"kaøÃv¿ä¬åÁX¨¿á§@¡/å÷¿ç~Ò£¦bÖOTHERunk1RXS J140629.8-652251?ÊÔ§0_üˆ?½V1¹¾C?z)Íü÷ž?ql­
†y?é'—îÛ?½²ÙÄ
£õ?×Õ.îZ¡†?Ã
º—"ðå?rZ0vé?ƒp€#øû?ãð´(¯Ák?Âãu£Ú?Ö¬Žõ¦Ó?°#¡'#?ª¦+€Yu?ŠþG\ƒü?ã´ÕÍ&ÿ?¯ËæU?â\—ë"Ó?­Ê$…Ä;g?05iº?{ûL
ä	?Ú]N}­ô#?­Y£6ŒY4FGL J1420.3-6046e?ꝁºÍd?ÎÆŠÖ8À8ÄëVûÀ9CQÀ¼ô@$ýýÇ@œ?ÿºjyñ]¦?x´u4ß5¿Ž€ÚZÿÕä?áÉD6¶Ë@
1iEhêпÁ<õ(áu¦?ÏëIúõÕ¿æž¾°nÈ¿åæŒÇ#? ¿éQ%Â1hX¿¦ÀPë!OTHERPWN3FGL J1420.0-6048HESS J1420-607?šM¸úôi? Å@p¹e?X.)D9÷š?k¿sÚ倢?ï#®}–`?¡üõ^ÝÛ?³ìñåÊ?¾7xU¶§&?š©Ö¨¯E—?¬Óç¡€w?ìÇ3¬}âÛ?ÀèWÞg-(?ÖYPޗ?±ñ¯á-o^?®_NÝrl?›È_†uE?âíb¢ÝT|?²r;{ÿlŸ?u7<¸"x'?qÞ©i^˜ú?uÍüçþÍ?|yf¬k?ïªqê•ë?Ä§c`w,4FGL J1423.3-5655?Ý:FÝ"/@
Þ軶$À9ËýíאÀ;€Px@Â.jÑ@´€Ǒ?Ô((}¢˜?á°:Zná_@	3ä%®æ2@9q‡VËê?ï¯oYT/,¿ÞÀ£ô'b¿ê_$º|¿îÚ®/ªè¿ïâô˜VN?ÒÐXþý—OTHERsppSNR G315.1+02.7?êÅuyoTo?ÀâaڒÁ?«z;oq?°ÁxÄðÌ?¼í¥¦$Ô?¹3–ƒ×?ÎÉ^
RR{?LJ&̎xê?Ñ^ėí>ø?Ë[ä»°?ß<Œai—Ê?ÌN[^=pŒ?Ö%ŠpYK4?°K^ݐA¹?Çð&»Þš?­þ+™J_?Ýâl|HÅ?±\5¯Ýœ?¹Íw›  —?šX¢.Í?Òi•còt|?µÎ|o—ÿ?㑆Z'±¯?µµxoŽ4FGL J1433.5-5457¿ïÿ÷Å¶@ @¿ã°>À9â2²Ú³?À;šÙ¯3^Ò@)áҏi@5%£þwj?Æ©›o\¯?Ög^~:˜'@Pu-©†w?úX×d«PP?ÀÆtÙpÊ¿ÊýpÄ
`'¿çÇ}³^g¿åWl˜¯ŽÎ¿ëi…ÀçÇ¿ïúñ"l'yOTHERunk1RXS J143329.9-545931?©~¯ã0ä? v"öZ™è?Ï\ðæŠê6?ÁÀœÅÜ Y?æØÈ*73?Ãdnº?´ÝlÛ¦?±>¹Ø$þH?Ùè4ÄÊî,?Çd:Ò5ÞÏ?àpE-u?Æ4'ý?ȝ@ûX¹?£eN—U?Ï64F¤?­s88x?â-Vî4)?±NNˆ?Üü?µUõ+Aº?'/Fïfä?ØGˆ/Öì?°‰HÞ«Êû?á1}Wÿô3?®î0tBâµ4FGL J1435.8-6018?ÊÚrvX搿"`Câ'íÀ8†µò•´2À:'s‡Ù~@Wꞙގ@Vžh5s?ÇrªÂ`ã?å.J€¬¸°@÷jrd¡j?þ%J~¬-?êYà[DŸ?˂&¶M.‡¿åŽÓ朂¿ïQ¢£Y6¿ã3*š}£¿ïëÊSuÈÚOTHERsppSNR G315.4-00.3?œO0>L?žs{'z?Ð	*¸ÆÌ?ÈYÂÀ¥êÀ?çøh±<?È£*uhðÞ?˜öqOûÄp? ÝMò™Ûö?×n¥KÜ;?ÍÀ")ǔü?㷕"Ú3¿?ÌÈÜö5ïB?³O©:Öíó?œö™UUJ?Ï(͟TT?®À"Ý¢§Q?åË×pЬ?°Æö"ãú·?\D-`HóÇ?M"ÝçýŸ?ØiP+£'ö?¾ïÛÒåv?ã½5Ó~?¾ði:½"4FGL J1441.6-5951c¿âà7Ú{¥Ø?»AV¥O°À9¯ñŸ,ÞÀ;Ld\ ë@î«8}tö@üÂ]Þ?Ñ+L§?ïþ"ƒÕâö@Ù"d¦@Ö m³·¨?ê®=Ë<©Ô¿í'úðÍ¿w%¡'ϱ6¿áY¥-Ã¿ïüwêó(¿ïàzßDH¯OTHERspp3FGL J1441.5-5955cSNR G316.3-00.00?²æ¸HD«q?±_h€Ñ?Û¿8îÌkA?́£À<?߇ÿ"iâ?ÌÊ]VH°"?"/½£Ðkå?œ©2
R?ÔŽºñŠ?ÏgÊjb?åXõK"Û?Ï[gL"éý?Ç¿ùêKõ?ªGË)ïýú?ُÅ9ª]?´¨ÙyI…?ڑv½Ñ/¨?²	x¦Hñ?‰ò¿Ž[?}´	s"þ?èՕ7[?½k¥Æi?Î}²»â?¼Ð`\ÃK›4FGL J1442.2-6005¿â5M8m¿Á4¾x¡&À8pM'iÒ,À:'_lw! @¡…èÜÎ@Èú½ ßß?½Vx¡k8ø?ÒCf;ô!û@‡ÑÜ×@"Üî^B¿ï§vÑîu?靖¿µ¢¿ã'8Â>Sx¿å"°üŒ®¿ìÒÔMʎ.¿çÐV#ùŒOTHERspp2FGL J1441.6-5956SNR G316.3-00.0?§³ý~¬ÁA?¡Ž°â=ù?ØÄ®`Gæb?È6£;kUå?â"h÷ñ@»?Ç̾Égf?£Qïõý–€?§Ä%1ԋ)?ͪ
Åóê?ǔJDziÈ?ç`Yý.©ž?Ç¡W8¢2…?»ˆ;{È<?¢"äÃ"þ?ØU|7þŠ?´)rdŸ?àd5ºt‡³?³í¢ ¬'?˜íJ›í?'ö\É[1?½Ý«}LÕ?§eM;¿•6?ëƒÃ&vý?©~‡Aä4FGL J1443.0-6227e?Ò0,ù7ºÀ.>ìÀ9})ž^û8À;ŽÿӊV0@$+Ö²ÿœ-?÷ƒM&ú@?¸Õp_c'Ì?»"™T¥HÏ@X¥H#…@@O~JˆºN¿ïü@ø¨ž¿äpaǛ4¤?ïû
˜	v¡?àÑsZj¯¡¿Ê[Ym¿ÆÞ°zՂOTHERSNRRCW 86?èŸ×5bº?Äñ'f·C?`îà{Å\?dkˆH2Û?Í<ê¼p†?Äæ6ºá}T?âl·Ö"¢«?ÐzoœßPS?o±:œJZ·?ž÷0Cl?Úç-ݞ%ö?ÐKˆ€gí?ãB»yçw?³ìö‰?AìYÿ?Šè·ÌŸÙs?Ø[Èö'!?²Pzx*?æ­¶×ɦ‹?º«dpÛyø?ƒ¦ð5'rÙ?…SçÕE?ÒZÎÀT?ºïÞzô…4FGL J1449.4-6026¿î|Š(§,ï¿ê]îBhZ\À8ÛM²:zOÀ:dåÏ@"'^±Ž@ºZƒÚ?ӛÍÐeß?ÐÆ÷ µí@ºç"Þ÷r?û…K'Mð¤¿ïÛíÒ?î@œ<âž¿è÷ŸsÎ-ö¿ê^áÂ}=˜¿ìÕl
?ÆhڟsMUOTHERunk1RXS J145023.3-602718?ÊJáWò#?ÅÀH›hˆ?¶ñ$†AMÜ?¸~_›1?æ#;M?Ëä›%§+?°xøEfãÐ?±Àån(?À+¶
Û,k?»9»ð?éåósÜXk?Á …ßõ:Ð?¿Ä'P}?'ü`ðÄ#?Æ&?Øh(?¨pÿL=?Æ?æ}Ýßúf?¬Ø»/¶M?¢U\!ËÀ%?‰ÅPãx?¹¦Óκhƒ?¦…Lw ë?ë¥ÏÄöî?¨°à²ÈÎ4FGL J1453.4-5858¿æPÁHµ%'?ÐÏ)~(¤åÀ8ö—¤ÌӃÀ:Z‰%®r@åÀb[>ë@"&~ïÊ?Ëç€Ø,§S?¸MŠÞ|ô?ðx×ÒºL˜@ZÌ´ùòJ¿ÙèyÑ}5¶?ÑUÈôÐ÷Õ¿ç¦G'Jˆ¿èʑž£n°¿ê €¾Z‰¿Ëºzå¤_OTHERsppSNR G318.2+00.1?›X›|¤P?–jšæó¯?³ÁçÉ?"NŠ?7~Ó?¡Ã"ZoqF?·"Ì
û?¶LóøG9W?›S²Bß#Ñ?£#.Ú2±v?ìAì‡Æƒ?¸?_ ²(?¾Ë_Ar? Üœ"32?¸ñnLîõ?ƒõ"¿Þ?éfN[óß?¦" Š?¸ –µ¯?žÚZyi?'4?Xl—€?zëõÌyo?ìj\eø­? 	T=²×e4FGL J1459.0+7140¿ïú?iLtÎ@E
c
'SÀ:*ŒžßS¸À<¿45'²E@"w¡ÍÏ@œSE!rA?´Æ¨à"Xß?²)"ø‹?ö³#ä
Öô@mÆáü3î?ÞKs0yD¿áÁ~_¬bõ¿æ|yÞ=bŒ¿èL÷à 灿ê¯þàÆ(ï¿Ù‡÷%ÛOTHERcss3C 309.1?ïè Þ¡Íñ?gv`#ô ?Kä+ÕêHJ?DÝ,\íÚ?`æh·}‰?f–ÅåE˜A?ïË̏'¢?~–Qàå{ð?6yÉöÿÚ?O[/&Ö?x²W&¼¿?|ÒAÈÐ(?ï>qCÜ_8?<ûå
¼?p¯·îAù@?m£^ÖºL?"éˆãšs?yÔH«Æ$c?ïøÝá× š?;K:ké!æ?2"èþ¿Ý¡?#7¿Ë0"?Cw$§&?7?ƒÂ>V4FGL J1459.0-5819?ÆdàÝÙm?߇ø\rœ«À:Qo'TÀ;ü;ëh™@ÄŽ˜‰¤@9&Ÿ¦ùÔ?Öÿyvƒ??ïÛ>w‰ú@
q#ˆY@,©óXý?î@Ôqü™¿ïÿÏX˜GŠ?ïýP 슿äÉ>$'ý¿ïÿü¿ÙŸC?ïÿ•!îZOTHERunkSNR G318.9+00.4	?È<6Es?ÁŒo¸%.‰?Ð<ìï=£?Çv6Q^?áÒ{÷lÕ?ÊQ«1ê•Ì?Åû$ÎFÚ?ÉEî…×n?Ü"BHê?ÉcÐ"á?åØ8³ûÜ?ÐJ²¸'?×Ò<µø¿?¬"óÄ÷|?Ï0"#W?+?ªÅ—²¶'è?ؕ«±žg¬?¬Žvã?ʔ¥¹8J?·öbíkÎ?ÛvƒŒ|‹†?ȅwPê|?×?)–ÿXV?í5¨ƒO˜4FGL J1501.2-6624?Ó䏃ÛÀ÷ /µÐ1À:Óúœé°2À</†K<@F6­;7@³©ìiJ?ʈüˆý?²¬¿¼°?ì‰8ž2Z?ÿ<¾U¼u?çåWr­œ†?é:ÂG¸¦¿é6Ä¢–¿åË·Ä'Þ¿R'4wU÷Ù¿ïü« —OTHERunk1RXS J150054.2-662400?æ·o›?–çäF³6?‡ë
#ם'?'ñh³"~´?ÓŠ@í?Â[ñÃï˅?â/c>)dÌ?Ç-8£QI?h*5#
eW?|¨¶«_'Ç?Ûpågž?Ǩ	#?è_ctê´?¦Ô­"--?—pÅ©ðC^?°ù©Ë҄?˔YLîLÄ?¥jÄV'?ì5jg­›?ŸPúc¡Ù,?'ŠlUÍ?{~úkU"ò?¼_8p™€?ž¡=—®²ù4FGL J1503.6-4146?ß)ºâG;@->X¡UPÀ:ôx'Y
]À<_JÚåª@ <','Û@éLz,	?ÉVöœT	?'Ÿk¯j?É,{Éz?ýH=ägF?$_öŠ¶¿èfÊo${
¿rÈÕ`3
]¿çÛêw¿¿àŽn—€¿à`Ý?á—_OTHERspp1FGL J1501.6-4204SNR G327.6+14.6?ë¥ÌD:™?µ À–>‰?aAò	€ì¡?Uºx·Ðÿ?Á&…Éê?´ûõû	?íˆ,ÈY—6?±
lzk3?u×[%;t?"3é˜Äݒ?²eŒG€ò¤?°'üZæ_E?ímvK?•¤	{H?èXzƒX?rÙõRœ?²V^Vò?"·•ßÃ'á?ëe`¤Ê4?¡OI;ÎEA?"Öà…h¤n?vf§žè!•?ÂpüuLå? ÑÆÄQÁï4FGL J1508.9-4110¿ä´ MÓG@-F§&J¥À:ÝÿTßUfÀ<'…o@*@Kڔáy@ñã݊Š?Ò'™¢ÓÕ?è~è]¡ñ­@¶,ºs-õ@y,¼¡†?ï)'Dé>¿ÒփDm˜4¿à(֞椿í'Í+d2¿ïÿß^IâL?¼ð&n(҇OTHERsppSNR G330.0+15.0?ÌÒª
©?½œ[Ónû§?áýʍ
?Æ·"ùés?Ë6+°©®?Á¤NžvBó?ÑxÂagþî?ÏÞeªÆ)?☃5ÕyÜ?ÒM!o¢Í(?¬neÚ²?¾6#–ü?Ðl"nHV?°Ô'(¿Ò…?á0t>}'?³¬]¬"á?Êe'u_=?©°aÉ,žœ?ÃäÛfÇ°P?¤59#¦˜Ö?ä=¹šÛÜY?´Üì¨x±µ?Ë$>-ÈÞK?¯ú6Du4FGL J1514.2-5909e?ïÙāq&*¿óW"ëïyÀ7§È‡Ã®@À:ä¥Xê|á@!Á»¤[iˆ?ý<96's? ›ªãÔ?s©…ž/Ãw?яãÉén@KûXÑRn¿æVc"3Öǿ䭕X¥´¿åÌeÔp/=¿ÔuÜyh¿ßÍ܁˜¡¿É(èÁõÙ6OTHERPWN3FGL J1514.0-5915eMSH 15-52?âÁ²ö–¥(?ėC•|O?t$…?q¼¤ñ!°?Ú,	²¦"›?ĉGº<—??Ô·SzÛ­4?͗ÄL1f?"æ
d+áÍ?¥ø¿´F$É?äý%×pÊW?Íêؑqp?ʺ´ÕGïÉ?­4Ö-]á?ªÿN3RJ?"±Ù>ÂS@?ç±ÕÊÎé?®h€Ï?Ûd'Z'ŒÌ?¿3LñgWá?·ˆoôI¾ý?­H³IÊ?Þ¹R¨Æu?½ÄÄOó4FGL J1518.8+0203¿ç‰ Ýñr@G]{á!îÀ:¯c>"¹†À<bã¹x\2@NóÄÞ@è@,¢Ûa»?Ð2&ìS?Ýï!‹k@Û·-[@9È"Ãú@¿ïÿýF\I?ïÿíUÙPi¿à%>þÃj¿çÑt!N¿ëçÇ$_¾¿ïRþª•jOTHERglcNGC 5904?穓e{&ª?¼þX7•ÃÞ?Âw¥¸^½§?¶9	Ëq/I?½ÄciOd?±!ûk´´á?èöéŽßK?Á֜¶sØ ?½ *^V©»?ºÈ¦8¡'é?»/FU2[î?¯2В…o?æZÑÝX}
?­KLÖHö?À¬&Þã<?¡×½¸§éò?Å葫ºnŸ?¤‡|Q‡2?ãðæku…x?«'#ñ
ë'?ÊK}6[$?©¿s,Z›O?ÅðéBóŽý?¥;ѬDD³4FGL J1528.4-6729¿ïúéâÿŒÀ"X%[À:·ä‡ÔuÀ<qfŠx"f@!
Œ!¶Þú?ü¢î¬ñe3?ÈZKæ]l˜?¿ä†Ò… ?ú0– ÀÕH?ö¿Ê"xzæ?ïþŽø›ˆ¿ÝLr^í T¿ãÜT)M¿Ñ¹Á¢w8ǿݬðäY0s¿á$I@:ؙOTHERunk1RXS J152815.0-673003?åbg㖧
?ÃczщŸH?^]¿Šî)9?V\¢#ÛF?ÕÒyGý?ÃWføÓê‹?ÕGøƶµ±?ÅÏHWŒß?†Ñ¸¦ý2­?'aÃ"Ōö?强°\?Åìׅé?é²Fðí®?§¸Ü¥Ñ?‡ÕúÑyùo?q$›äXƒ"?Ǻs7$©°?¦´æøZ€?á׃r91?®³Ð¼Wo?©ºÀdàÄä?—xÈ\ô"$?Ù¡ñ…3?¯FPkÃ†4FGL J1533.9-5712e¿ïÿYõ׿ïÿ"ÞïÀ:°ßé	CvÀ;s­íät‰@(ŽÂ¦]¨?òUav<??ÕÂZµX<?´–ÜO÷?â	>m#
?ô´ù[öö¿ïÜb¦-¿ílÚ>$}ä?픁+äŠY?ï÷ÂCÜΣ¿ä*X-¾,?Æ%{º‹©OTHERSNRHESS J1534-571?ɝÿ¼‹Áý?ʍAZÚ??ŽÎ¾…ð?E¥µ:Á©?锎7Kñ?ʒƒYz®b?¼v›ö?Åùñ£Õ?Ž {¶g"?¨ªÉ£"Vz?ì/=·¡ã?űK¢ÕqÊ?Ø56в"Í?±î՝]¶Ô?¥2Áªù?"
©¡·?â'B®ššê?²!±ß¿[?žéÞG?˜â"	­ôF?Þ"ã?sф¤?îÈõšU/? H/W_ê4FGL J1534.7+2331?à¬uG"@J‰,à2ÛÀ:rÚ:s™UÀ<t¥µ0Ï@£àE$¢L@YÚakU?¾/$…ÆS¿ƒ@f«
gû?ÁÃì¾Ú›Â@y͸/0ð?™t6!"èD¿åaþÝÁ׿ä]`='l¿æ·a*½Bì¿èÀ0§g¸v¿³XƒàÛޟOTHERsbgArp 220?ïJE˜¾•©?ˆ '©'T¤?uGX<>Lþ?g8ñM-a?'evÙ·x?†#—O9"ª?ïœélƎ?†Â›³"a?Cø²‹ß?UGÞšëº?‡‰s'Ñ3
?…¡ú™‹Ê?îØõp@T?…‡€dh›c?sy8^d?a™%üç7}? i9=?ƒŽ(e9§Â?ïÿ$‰þ#?n1Ië?j?CU½',?U~ò#q!?…pf|?i¿4t2Œ
4FGL J1544.5-1126¿ØÙ'ê7@@9&A³À9=ì0?bìÀ;ÈRÆvq@âd¬'ä@5†S€?µaL̆Ç?ͽyȘá@ºx)‰‡?ú¡®÷Š?ïÞðáT[¿Úiþ Õ®¿å®í¾´Ü¿êy…'ͼ¿êlH"ș¿ïɞs`JOTHERlmb3FGL J1544.6-11251RXS J154439.4-112820?ЖÛ2ÔÎ?À©=ä?Ó¸?C4ò1?ň'^úþ?Û°å‰öï?Åí=À†Wì?¹äÖ^XLæ?¸^Onsõš?ê®n–Ð?¾kÀ1€¡?°§´íŸ¬š?§Æ±!ۖ?ÝE‰\žš?±¬ºÌž<?ÒNlu?°UÌ3N¤7?и!^"ôð?ªÚþ´D?ÇDlUé_?£((NãíJ?áυ'¤?·Ñhó	ìY?Ò\V?¨?²úï"u,•4FGL J1545.0-6642?§t[ä°­ØÀ"ÃH² yÀ:L÷z€ÏÀ<Kµëæ@"!N"b£
?úÅva†,Õ?¾dZGŸ&?™p1ãŸCŸ?Ü˞":ê?ýà¸L7;+?ïöD_«aB¿ìáT™4¿áW'ÏQâK¿ÕHd]L·>¿ÃLu9_¿Øõ…ÞPضOTHERunk3FGL J1545.0-66411RXS J154458.3-664153?å+)É"†À?û£)Ö?t‹m]¯Ç?eî=%r6Q?ÕW~¸Fƒ¿?Âü½*67~?âuæŠ6?Ɇ«&6à?jU[~hx¨?zÈË0B?Úá{îÂù?Èç5¼f
ó?é`¹}Î?¦ª0è'Ø?†÷ÝÂòq¼?n÷Ô@à9X?ÈS°êá®?¥ÌŒ??è`2"'Ô?¬ÕÃ}m%?‰¢ÈôÀúÓ?XÅâšÒ?Ìå
ækµ?­£§sYìö4FGL J1547.6-6601?ä!w
<]ÃÀ"ì·M߇À:¤W‰SÑ8À<òÙ¦Ïã@k\æàÊ0@¥2.?Ézô'äs²?±óy^æ•K?é—tü+@áZº5Æ`¿ì"Ö@éÕ?ï÷_²íþv¿í°Ú'ÿ#¿Ô)ªžNµ¿ïþ;âÐ?ïÚÑrMû6OTHERunk1RXS J154730.5-655754?í'D'T?¬vIʛ#\?‡vô›=ôË?…7€Ð…÷?°ˆøês¶¾?ª"HÀöÈx?íça'ƒ?¸×ÀD;òÛ?R¹;*O:X?mVìðH¹?°|>¨J7?¸«È…L¾¹?èµ>¿_`?¦è}6"?¡@Gz|(D?Š¾3?ÈÚó#ãu—?¤Üe$Qá?îÝM'+ñ'?‹»òÉáŽæ?|ñö\W%?qTîԕûæ?݃lÂ?ˆ#ߋ|1á4FGL J1552.4-5612e?ë͏¢AUW¿ûöŸ™ÛÀ9Ü'³£0À:úZiØá®@!8X"UëD?ý¹á7½Üo?Á=
w}:?ÅÀ=\×ÇR@º.šG>ƒ?ó/ëb^?ïÿÔač¿ïèë Í?ï1}ñf®¿ÚTÁÔiy¿à&ǟ¼Hp¿æÞ'h#ÕÈOTHERPWN1FGL J1552.4-5609MSH 15-56?ڐ'ã$?Ëql´ŽÑ?‹À)^•?Š:š-X&Ô?âH·qÎ??ËmŒÇ™…?ÀÒøËÝ­?À²ÊË\á?§‡ ~Æ®³?²woµ+S?êRÇóà©?ÁRäæ?Ñ$6~q]?­:RZ-<??·"ÜG.'!? úÓåÁö·?ä}d[Úõ?¯†6WM(?®|@™_ÒN?žäq–°?±zqu¨/¿?®E
5jáä?ëèíÇ´üã?²ÿš¹×4FGL J1552.9-5607e?ícýéqÁ¿ûÃ"›5{À7ª·Üz¿ºÀ:RŽ¨¤ÏX@ –=^…F{@¿Å¥'¡?«`Þ"J?µ(™QJJ|@È7 €=¨?ôý>!MØ{¿ä©»Þh?ïÿ—Ôú¿âJq=Yý¢¿ÞF™!N¯;¿äÒ,ó~~¿ßŸ[O7OTHERSNR3FGL J1552.9-5610MSH 15-56?¹
ç+aË?°¯Žfqï?¯S­:µªS?³ß^'ÇãÔ?ê鄏o9"?½M|!?¢ï<cŽÑ?¯½9úˆA?ÞA鵧¡N?Ñ<6ѝ¬Ø?ß{øbËì×?Ð/À¥G?»·³/YA?¢Ö(q5‰b?¹Æ w3¹N?¡`Œ8_dŽ?éWú³­?ª¿D?'äD†¯H?|xÛêæ"?ÓérZÂ?·Y(L™Ø?åt$®ix¿?·ºr&.C54FGL J1556.0-4713?é™MâiŸ´@EUÅ.rÚÀ9F"'AiÀ;.…bªð@Èӌ.¡ÿ@K¼±Ì–F?¼ueáÙ?™:†¨j?܁M½£7?ä;CÖw#+?ïÿý{ÁA~¿á[?÷fÔJ¿ëwpåEi—¿èVÇ¡Р¿àãÕÈc¿Ô‡^ƒ˜üOTHERunk1RXS J155608.6-471529?é@vC4w?ÇO†"¾¸Ä?zœçíþV`?xY/lƒ?Ê)@·ƒ;s?ÇZÆâp?Ъ¬'1ÖB?ÆknÝ´ª?¸ìS£?¼ªK]ù(º?ä)ü ?ƪ>L<Þõ?Ü.ÙÁ¬ºI?°ösãån?®èŒøŽêx?'".4 xÌ?ßôŸAhg?°?kˆà®1?Ȃ\¹{ŽÞ?ªBÃLÎ¢?Â}L¦6]—?ªDʛ6¡—?å@¨"ã?³Y¸ù¢,!4FGL J1601.3-5224¿ïL/lîڃ?ÔÓëd'{ÃÀ7øKZqežÀ9ÀBHyìU@^¾†GW@løÿZ¾'?Ã÷ÁÃuU?ßó†?IÁë@ÖO@¯óx?úŠ9\mT?ïìz|àP¿Ñ¾²m{¿èYüá¨I¿íhåf÷…Þ¿ëf`ۍ¿ïäèaþ¢³OTHERsppSNR G329.7+00.4?©"­ïÈ&¨?»°êa>?¼‡
x¦_?À2 ´‰ó?êÛä?ThÊ?ÄÑkº
?Ž\¾PTÏ;?–/
8–'¶?Ô瞃ås?Çæ…Rë?å½Å:º
?ǟf導U?±É"
Üa$?š°(URÓ?Ñeôäy?³ÅÜNk?å7Öªž?´\`"1U?@ã|º†åw?/'ãpqŽ?Õ.^I%ø?·‰CHŸ~?åd—ü>b?·ŒF+'öÁ4FGL J1615.3-5146e?Ì ä(g¿å3X ÈÀ7ØÏä¯A¢À:o]Ø"ke@#.zìu†?ú#'ǁ&?²¶""Ý?º ~"¿÷@
\irŠa?÷œŠÂ¼'¹?ëWË-\¿ï";C¢í?ïž%"ôÆç¿Éf8ِT¡¿×æø<g9u¿Í)- Í›OTHERSNR3FGL J1615.3-5146eHESS J1614-518?Á''Žo'?ÄÃMxcy?"`(ŒŸ×?£<ÝÝ7›Å?êü{÷gÉ?Ç^ì¶éV?¢<3¸x¯˜?²f~³ÙÆf?µûŸ•3Á?Ÿz.ô¾Ñ?ìÈÑÒ/?ïeóçû?¿W§ö?¥XÏx˜F?±Ø'†jx?›xx8X
?éâ,Ž§»ì?ª\Há¤&?'äïö¶?‡ ¥¾Â9?¬çAVˆµ†?ªkO«®¾?íšdjáÄ!?¬Í£c¤4FGL J1616.2-5054e?阶ÝC´Ø¿À©ˆOnÀ6â1_ô\^À9ÎÒÿì´Ê@!®š‡«/™@aED­®ú?¡Ùt~Þ$?'¾#3-K_?á¡_²??ühˆ_?îï«>\²?~c45oV-¿àŽ·ó÷´¿à"pð›¿äÓgÁ¿×‹&ŸÇ±OTHERPWN3FGL J1616.2-5054eHESS J1616-508?–÷IJŒÄ…?Ž)_U
Ös?h~ðàs?p'˜Bd±?ï/ÆĈh?àtËû´? <²7†H,?£BBö)b.?·fR:áù¨?¿	ôl5îˆ?ìj•+\H?À@_Y§â¬?®þ²[ÅÊ?—ÏÉ28UŠ?¤9	$AF?ŽÍa8«‰?ì̄E÷ÿ?Ÿ›} m/?›Uðh	u?²*Î(üÕ?À¶USv_G?°I+vƒž"?ê÷»&7'ã?°£Ù
U4FGL J1616.9-2257?åç)"ŸMt@3|€Ç:¼"À:GOµò–À<	÷´#ì@<r¢ÿ@gy¦µ?ǔf'?Õº´|ª@Ú<÷Ø?üdî—!ð?ï÷n@ÐT¿ät<Ëbj¿ßÔ½|Lן¿ßͺ}¿ÉY¿îZŽâ™¿ïÿÿ)@k*OTHERglc3FGL J1616.8-2300M 80?Øö®9ÃAa?Ä
å[&ö¥?Ý["š‡?ÅÈËçˆ?ÃïìeDo?·'EK슠?Õ%ûÖÄE?ʾ"!œnF?á2µM?Î5cM¶Ÿ•?Á§=ÇC^?·kÌu?Úc']áÈ*?±U˜ûí3?ԛŸ~ò?²€°>OU?ÑÎ#,&Ò?©€"ÕÒ??́"š"É?£E{×ÒYü?Ôg0ËÈZL?°7'­@«ê?Ý
qêcQ?®{ۂ/4FGL J1619.8-6314¿ìÕضSÓVÀ"‹<æÀ"À;N»"¥íÀ<¤$Ÿòy@!ŠÙb\k'?öhó ¸r?ÖuK[žn?Úû•!ººÑ?ù¢aôçž	@µ'§‡ÃÙ?ïŽ^g"cпíÉ_²¿êsŸ¿£n…?á¹O!P\º¿Ùâ`ûÈ¿âU1U¡ÏOTHERunk1RXS J161946.9-631530?è×û°×¡4?ÂßI>ØVñ?iiw·ñ?ë?Ǿ%?ˉz¬™ÿ´?³8ÄÎóz?àtΆ?ËYŽê™?hü{É©jn?{‡)žY±H?ߑl2ˆ?Êïa™'÷@?ê#\Ð_à}?¦ÑkÒ^?"MÖ\ê~?'8ΚC¼;?ÄèÑûTà»?¤)ZlÉΉ?ì´BûzGJ?¦ÄPÔÔ<e?oÏC–J:?sl¾CqV?¹_p"c?¦x6†Ú]4FGL J1626.1-5904?åÏò¾p`À¢	?Câ®À:Ûõ ¨ìôÀ<ªŒ0$‹@ Xs~@©ñ…é¹m?Ãé§c†¸¿¦±€Á™G?è<ÓÅåR@ïÃåG—ï?ïÓýB¶]õ¿Ü¬3$D­Ú¿ëÓ	\ ¿èw~¶ß%¿Èäß¾%±?–''ᶶ,OTHERunk1RXS J162613.6-590658?áI¯¡DØ?Ä Xdñnn?‹¬@ؗ5h?'GÉTËQ?܏>¶8¼¥?Ä¡l!Y\Ì?ß3B¾õø?Çs¡ÂöÙ?pȺF‹ßh?…üwY}²
?àDÍ+øcÆ?Ç:AÁZØs?æüÿîeòv?ª¼W{HUæ?—@"Ây͜?€ú j9U?Бý÷~7?©Ÿ™	8 ?é÷Iê~Ÿã?ªÏ •cF?pcZH/Ð|?kZ'y	?ǟ½ƒÄï?ªÇ"IÛ¹4FGL J1626.9-2431e?×Bׁ—Ö\@0º{¢7ÍÍÀ8.ΉenðÀ:¾É'•q@ÅÍc ŽU@ÌՀÐtø?°ú*~å8?ºãi`/¯_@šÐ=š•B@oXiM¡t?ï¦qï0¤ã¿ÚðŽ•·¿å,¡^4׿äL-ráõ¿æj#?O§¿ì½¸ƒi¬OTHERSFR3FGL J1626.2-2428crho Ophiuchi?ښêÆü ?ÄÎÄÐB)?¯ëOš3?¥€"MCu?àÂ<;"Þ¾?ÅU^j <&?Þû‰‰'L
?˟/^«D?ÙÂ>­f?Ìz‡®âÁ¿?¿ºÐ଎@?²-eˆõù?âKló½?²À]è`B?²!}Acb?šÁˆì4•?ÖàÈss1.?°ž:q7J?Êù•öLHI?¦¼_¥o‡?ÅenR£L›?£V"3‡Ò^?ãè>íÄÇ?±J,Ô)àÖ4FGL J1627.6-3852¿ïß[Öљ¡@²Y@ãõÞÀ9£.>׬$À;‡A©î{s@•Í`E@¨@ƒ}Îb?Á7úÃ*6µ?Àž}5ês?þ•Âú»óa@8þ'¢?ïþ0O‹Y?½ï¦–'7þ¿äAç`ÌÉr¿åYg°ã¿è›lØpnþ¿ßgÍÚmOTHERglcNGC 6139?Ø}ØÛº??ÂW…­F¨Ò?©€!dð·?ØÈÉX#?âÓǑÊZ?ÂþVz;EŠ?ÚhÊ;›Ã<?Ɠ'v¥Ó?¬iíy=¿0?°BiçÇ|?áü
žBo?Æ ÄßR[ø?à؇–Oë?²@Í<øóN?®SôŸåK??'üã¿õ]?ڄsdÖ¶Ã?±Rõ-
<Ò?àŬ¼	¹º?¨à¡ۗN?³Qê<õõ?"ÒÈp½Ê:?Ù ,O?§K/™³4FGL J1628.2-4848c¿ãa(µ£2¿§¦{ªEÀ8ɦ¤D‡À:>žm=ðü@7RÅʤÿ@±y|ßý?ʦE9'ô?Ûß°i¿·;@'mŸ?ËÈ?ø2·bWc¿ïM:'£?ï­¨z-¿ÃœÏÄxëN¿étæX¿î¦\?ñÝ}¿áì!%êuOTHERspp3FGL J1628.9-4852SNR G335.2+00.1*?p'	¬üa¨?drÃ	oqà?®;Å¡Ñ??«.gQl\?íû!'ˆóE?«ÉƞMa?‹¡ÙÓ¡†?GNø?ÏЮŸ-×/?Ĭ¢BÛƨ?çOøÍ;¯?Ä}ؔÈR'?®Fßz‡Á?lQêÌ?͔>Kp̲?®'¥I¤»±?涂u{PÃ?¯.ª…åê?s❹]å?`Þž`j/?Ëv¹-÷´à?¶=šÚ?èúŒyÚ
?¶m@íw÷ó4FGL J1630.2-4347?ïc–H½oH@	ƒÏ:eVœÀ9ÓT&ÈÁ¥À:ý¿;ÒE@ )f*×D@«Ænäº?À8ò9î¹1¿²ÉÖù "?óu­+FÕ§?þZ¿êU?ïÿu+%G¸¿èZ&–m¿êzÿzŸ¿éŽ!€Ù.Z¿ïá0œýç?ï"Ic `ÉOTHERunk3FGL J1630.3-43461RXS J163023.2-434804?ßð¹'&Ó?Ë_½ctÞt?‹_E£?\÷÷3?ßÁ@ä~ü?˄¤qK=ð?Ô*(ÙITÛ?Ê(œÑJùŸ?¡âË…<?ªWfîb.?äÌÉö©­??ÉÁ½ê&l?ÖeJ[¤e?­ðÔ?¸˜uP]#?*,±Ù±?áòÚL(")?¬Ù«cú&Ð?À^†¦Ê>c?«."I!Ë?™›vLdf?",!¶‹p?ëÉz›
C?®+Z·ùÛ4FGL J1631.6-4756e¿ïÝ@àšßë?Å>ÜIA'rÀ8;i÷ë^ˆÀ:,žh5s@#‡QàG}î?ü°œ!3?³¬
åpݎ¿›äÚ5+¨? ®¡>@c#ÃԀ ?ïÍÐmk=f¿ïý·áXJ?ïh_/:€/¿â;&a"˜Ï¿Ü³±ÇP·¿Ã•Ýað_úOTHERpwn3FGL J1633.0-4746eHESS J1632-478?¶a59™?»ÔöµU	?lîçC૤?}ôƒ~R3?íêqš¡?¼…8בný?·è[n﷙?Àˆ.K^?z ™¾<%?'`XŸZ¶?ìγ^¥Ä?ÀÐÜ_Âö?Å¥¥U¹I?ªb!'¸?­"x©‡?˜6$³P	˜?èÅQ"Ç?¬í
åK?¡K Ñì?"ü0éͳù?wÂÜ(Ÿ?z‡ªÍ!•ö?î»ÉÊÈVB?–$ðP™þ<4FGL J1633.0-4746e¿íÓql(ó?½Ü—Æ܉À6 þÊuÚxÀ8öÇÿ²|@ ìÒ1æ'@éÓHæ#?¥Ž
¢ÎÕ?®ôßô5¶@'Óh@bëà8du?Ü`àjcv?í¸Dµ;¶¿â_{l‡é¿â£-ab§¿äÜ(ŸÜSÓ¿âù ÀTnOTHERspp3FGL J1633.0-4746eHESS J1632-478?€½c"3P?y;ÉrQAç?"~æY1?˜h2³V:?ïkB À?šl}G(ú?'–#)§î"? ÑðŶ?Ð
îZÀ×?ÌÒ¢™y?ç[Çï…` ?̨0ã‰Üñ?¹ ¤õ‡'Ž?¢ÝõÒ¢@?±Ÿ§ié¤?™×zÓH?ê§ötÙ*?¦À&ééð?l‡€À¥?c%§¬'Öƒ?²y ¼Œ–$?¢«€Rë4?í"ThX­*?£0'5´ç4FGL J1636.3-4731e¿ã8äë|I¿¿t Ù¬"À7:¯ÿ6¬À9b>G]@ …†× @t[¡çEõ?¬û&Qxm¥?»%A>IøÙ@Û]9—?ÿ=lP‹3?êv?ø="ß¿×Á±[Xp¿å9‡
Jݿ䧤WÚ¿æç: ã$}¿é
ŠA·ÛNOTHERSNR3FGL J1636.2-4734SNR G337.0-00.1?oté?cÑøÃk?",EÞ¹|?†Œ¿+û?ï<Rän?‰=g²ÁÛ?€G¾Ö?'J?‡¬}Î)M?ОÊ´û@?Çèã¡wœn?çoÔL"?ÇÁþ"ˆ¹ö?¬©Ì.Xg?•ÚԖ¼¦1?·<^é®Å?žlÚ¼^@?ëMϑ=Iñ?¤‰E&V«?RªÄOt®Ü?B"Bó{V?¶hßgóÎ?›^lì-òU?í6ëG.?›EoéÇ4FGL J1638.5-4657c?£õ+A6¿™¬.FºN›À7´Ñk—ÿÀ9*OTÑél@ ¹ñ¨ÏB@H½Þó?þ?½¨K
DŒ!?ËE‹:_e@ŸwÞ]îÉ@^ìJìbi?îelZþ¿ä(05Qñd¿âý™ô2l¿æRɛ¿ä‡¿ê²á~µ'ž¿ïÕ)ÝÉõ,OTHERspp3FGL J1638.6-4654SNR G337.8-00.1 ?xˆS	·Ïh?tze¹7À?¸–Ön+ë?´É0|β#?켌'þ?µF÷Ò:?Œúˆ3"?"ÎQ
	$Î?¸BU¤Ž2 ?¹éŠl•à?ìƒÍÝ?ºNåo*4ˆ?±§¦@´??™?Áj+á?Í$ú&×ÔÓ?°"¦®ÄÄ?æÌ®GÔB?°Öåjà'™?FÀ½©¬¦ˆ??åO+w"?žÕeþg"?¦Íùò(?吝e¡™?òV>ƒäa4FGL J1640.6-4632?áy'ËçA¿•aÛížvÀ82]œ"IÀ:n­2ӑã@#L¥)DÇÛ?ým  ôØ?±š!(ïl?˜Aä&Ìn?àïJÀîr9@	'™oþ?澖stkã?äK'Iñ»š¿àsuã±ë ¿Þ_ÂWÿ¿áLʳíض¿½VtUè>îOTHERspp3FGL J1640.4-4634cSNR G338.3-0.0?¼Ç7<\@?±7Q|Š"?ŠN•8Ñ?Ž;@º«W<?ëýà­#'3?²ðØeEƒ?°îƒûc.?·ªgÆÆõU?'Ä~¯Ë?H…9–ž†?íTæ?¹ 0ÚvÒ4?»¤ŕÚ	?¢:½Í¹-?ªž·fÎ)È?"(§sd?êᐰàb#?¥O"~~ƒý?±8½v¹B?œ/!ÓWK¯?¯G¿æõX?¢E¢~†?ëèÃÕ*nc?¨C7¡­ 4FGL J1641.0-4619?æ *®ý¯?´J b5ª1À7rÀCQŽhÀ9hÞZ"Ê@Œ‰G.=@•&§3¶?±B€Ùfè?Ã%>¨Ý.o@¾Oá¿£@ø»h {?ïþ/°Ç³ˆ¿á°"Ýz™ú¿âžÝ¦8äM¿æ…~†T¿êDûbÓ¿ç|VÈc±€OTHERspp3FGL J1641.1-4619cSNR G338.5+00.1?ßìGêP?z•Ú\샡?§"Un&`1?¯;ZúÒ?îFZøjU?°]—¾¶˜?†íÖoZf¼?ŒcEnþ}?ÊQž.PŽ?ÂÊ{—b/1?éá®'?Âàˉ‰áD?³^Œ¿‰?œ¯puêŒ?Ĥ'x#"E?«3xº¸û?ès¯_FM?¯´94Bè?[‹¿Ý!a—?NÉo_ž`4?³xCÇìÆ{?›Â+ìp¬?íƒ1§ր?›w-ßþ±4FGL J1641.3-5945¿´l¥ŠÊ'À!›ÿCAžÀ:Jœúw*À<ëoOC4@UbPW0h@úp#~ŠJ?½¹¾'B?o3§ƒYi½?¯)9£P@I¤µ¬t¾?ŤĚúÝ¿æoû:ža¿ã@Ï_~¿åÐx=~e·¿ãJwB+ɇ¿ÉLáłU°OTHERunk1RXS J164117.0-594647?ê2!ÖB?µ^:\ð!p?é-ŸïDî?rbÑî0i?Æ6'Á,Ï?´ëÁiI»'?æ ZÑÚ?ÆÆû@NĬ?Y¿gMcK?mx'l`{l?ÓÚ¹Šö é?Ƹflõx'?êSޓQ?¨¼:vMŒ?'Ó›OÍæ?{úSÍÍn=?ÅÄ=¹ˆ?¦Ã[¸VÜ?ìØÖîÉñð?õ19j'?tÐ5Ëì­7?a¹~D†¨?·ìE,ñ¥©?'šÆòÇh4FGL J1642.1-5428e?벲ђÉ
À¸ñ.ñÀ8ãíóŽ¶À;5@qà,@"¸	ò=@÷`¤……æ?ÂApã—êm?ʳ<'è'F?ýÌ–›¸X@cbezÙ?ïÂä¾®&¿½ûå~ŸmC¿á𯕄a#¿éikž´‹¿à
Ýað`¿Æcê
J[ÄOTHERspp3FGL J1645.9-5420SNR G332.5-05.6?à…Éy5@?ÃÜB§#6?'Bï³zó?Is«ž?ÝÓ8ޚG3?Ãé ¨Ü*÷?ážÇßÏöÈ?̛ªü)!?šËHŒ0!ë?¨o3i¢É?Û»·Q?ˁð<ޟ?á(õŠ–C?´£ŠQWÛ4?±¶Áœ¤e?—ò/6U.¢?ÙB%䃪_?²}ŠoMt?ääHñ²ì?­ŠŠ"½ñY?ªüú@§vM?•QrPɉ?Ò×Îԇ^?«^Ž¼Ü¡Ï4FGL J1645.1-3323¿ïÃ%(Ùh@ÇäÅøÀ:b/‹ÞÅôÀ;ÇŸïôð@Ñ¢'dì¿@Ayaë­c?ij»¤†]?œ2EfUcN?Üq°œj"X@mF/9?ïìáxU¿Ìp~WÉÀ~¿éšÁÀ	¿Ý¾Ùå9*C¿Ük
…?›¿è\v"œ;OTHERunkAT20G J164516-331816?ãüçÏ@ˆ?Âv•C\Ö?'!Ûx|.8?yÉ}ƹ¨?Ù6÷T~?Âl¡E®å?àe{ìen?ǤM¾?ƒ£-ô°dò?'Ò3®qd@?ޗ[ü?ÇM±_âZ-?å\ÉXÏç?³*Î	­Jš?€ú<í	Û?†þ:ò3k?Óoèɏ•?±Ö³]€Aó?çær€G>?¦½Æ-÷>?"ô Ú9ä??tæ!´•ü?Ïëñ?ig?¦hò÷±V4FGL J1645.8-4533c?î#ïlp&뿧.€_ЎèÀ7Г¨¾Ð‹À9zc'ŸÐ@ê¶W?ö@DV;u÷Ô?À`"•N?ÐÈá°´"@àÀ_?úål8br?ìVP%"õ¿Þæ[L
¿åƒÚ_Ý`C¿éÉÇÄ¿ì/_i#¿è™¢¾[oèOTHERunk4U 1642-45$?yÏüÀpþð?|á'‰d4?–Õ¥Ûç?—ÑNŸMC"?ï²Ýø>Ë?›kÝýa=	?'÷Ï¥ŸT.?–¾²fþ,`?Ëõ²Y|Çs?ÀÄ¥_ë•?èrÔìsӂ?¿ê
3LÈã?¯BŠ3@nÞ?"ºhÿÒ0G?É//¯ÓJ!?©½	ÛTÇ?çÀp×&‰?«w«LP¨?RNàAÃÒ;?C.†)¨5?¼xF6&?¢·»˜?ìgƧ7Q?¢ÓDfE½4FGL J1647.2-0154¿ï÷K²·Î@:T;ÄÒ,ˆÀ;üè‹+À=»	h_@ wɉv`Ú?üó÷é±	"?ؕ";ᭅ?ïû³ŸÕý@ÏE™›@¥"ºÔõ¿ïÿÿ" 5•?ïÿò> w?£	1à€fu¿Â"ÏÅЄ<¿î/é¿ïÿ}e†mOTHERglcNGC 6218?ë8§¦˜M©?¿Á»¹XY?¾'ºJ.]?¸ÎÙ°_? d`!æȵ?µ5Nā£?ÑJå'?;,F·bý?äj[Jûª?ÐÜð˜<u¼?¸ú¤fÀ?´#qBù
l?çRIðV?±)µ®Ápe?ÂJK»à¸Ú?ªd:â<e?ÁtkۅË?¢žvI›Î?σ& ô?»jÍáõ?äÛFí A?À|or½Fà?º{Uò¼?ª'®2¸ g4FGL J1700.1-4013c?ï™ønçu?ôãŽ)ùΎÀ9+©EGÍÀ:´Zøt"@Ä=®·8@@›ùÆ*?Ëq†Àyt?àc!m8¿@âÊÿm3	?ÿEÚdåÝÀ?ïÿô!O…ú?Í°:ˆ¥Ö¿àý)áпö¿ë.ª¢ÖY>¿ébߓxî(¿Ýs—ºñƒOTHERunk3FGL J1700.4-4019cNVSS J165941-401121,?¾™ý¨ÚÏ?¾r±R.6Y?¸mŒc5vÚ?¹ÄqŒU¨?é1{3ä5Ì?Ěîd¨§·?²``+Ü
=?ºÛû\.Ý?Í5¥xÍ?Æ×^¼A
?æf®Ñ&~%?ÈêêsP*›?¾ú6†\zª?žyÇz(
?ÆÀx"ŸB4?¨2ª¥±?æp› ?ªV`½Ô?›
`ÐW¡?€ç"½†•?Ï$ '6ÇÊ?±%'T¹ƒ?çYï£+ËQ?±õµÖ'¯4FGL J1701.0-2617?°W0Mn«@#Q2rC{À:zÝì¯ÁÀ;æiŸ
w@o=O–Á@Ö3Îc¥Â?Äóöû‰#?Ä
‰w¹?üv[ÁǶ
@V^Ä0›ÿ?ï	GÂ6pÕ¿â
Fªß<¿èݘ—;ˆ¿Ö&ˆ_µr=¿é"^úŒN¿çAÀ>ÉêOTHERunkPKS 1657-261?Úg;"?Â;q4•k?¢<›¿¿œ<?–86×U¥?ᨮÀ½hr?Âþ±¢lz?è5v¨µÐò?Âúb‡C†:?Š	Þ6)ð"?Ž&F?u?͉‡yÆ,?Â^{Í.r?çxº&á+D?°ÌÈðCö? "+[Åu?ŽçÅB†ý?Íù¶Y¤a"?­ñ¹Ø+&Ì?éñƒÿß?œlúmÚ"Í?¡ˆÍvïþ?…à´Yä?Çb–'D"?›ÂÕ[Ê´k4FGL J1701.2-3006¿Ã+]¼HÆ@Jì$·oÀ8©2ëƍÀ;"'>E@V.?ÿà2Š–ÇW?°1§—ß]?؅»@]h;@&ÇH!Äv?ü^ÖDoƌ?ïþFA'×5¿ÓP&žzT¿ÝBã_5o£¿ä''wcå¿îɨ G³ž¿ïÿuᮆ;OTHERglc3FGL J1701.2-3006M 62?|)
1fuU?vtåÄFwp?륭l$˜Þ?»­²@?kä?Àˆýâhá?ºãá9U?€
Ã%ÞqÀ?'3{Àx!Ð?í¼ä&=Ñ?µ'ùªJ"L?°ƒ'C9?´#
ëƒÉ(?‰úםMð?vÛG¦[m?ìÂìX%(ä?8ù­B?¶´Ýãã)?›¯:¶\?cÌ!_¢"<?PæÀ±>"?ì4X.!¹?¡"ø&â?¾‡ü3'Þ? æyª½4FGL J1704.1-4140?å<Š+ßÏ*¿Æ᳤1ÎÀ8à8¦À:æ5SŸ@ lZ$c·Š@<å;X›£@ÏÓ¥."R?à/SàQäÏ@îÀrKv÷?ý'Êß·¶?ïöÉ™"{¿ãïD[y£Z¿âµj¿'{¿âŸp"§Êµ¿é¹ñÞ&Ò¿ïÿ2z¦KOTHERsppSNR G344.7-00.1?'þE1å`Ã?"l
¾äh¾?·æ.2x,?ÀÛ³¦ƒ¿?ìkKª…ô?ÁËHJþ‹Ð?°ö<#&>?¼Oݪa?½Ì™¢'Ã?Ä5u?ê'¥YfóF?Ɖ¿VK&Ê?ºÃۏƐ?™PëÇG?Ë×\;'ô÷?¯†ei[}ð?å±­"?°"ÈU/?²G«‰à{ ?¹ïN¦Ñ?'æ¬ß	}? Üœ']ßÃ?íkoÞttv?º¹'ï"Ì24FGL J1705.7-4124?ìäۖ$6¿ÑA…±ZÀ8q=†ÅÀ:ÅÒ݈@NQŒÂ@]lÝxì{?ÇñPå ®6?ˤK¤C@Ç@ˆ…ZGt3?û½-Dܨã?ï­tw¡!M¿Íœñ½Ç÷%¿åÈ
L4¿å@@aïß!¿èê'Wގ¿ïù+àŠðOTHERsnr3FGL J1705.5-4128cSNR G344.7-00.1?œI4í,X?"Ϫ~q§?´³–mÀSÊ?µœ;}Šôø?ì‡CŠÛt$?·®©*"¢•?˜ƒ®--?–¯ÂŒyýý?À¡®v'r@?¹ØJä³²?ë|Ȳ?¹ùß_Úl?·
xܘqŠ?™¤åÕfÍü?ªAªV?m?¦yÛ®V¡®?èsÀy×aó?©rç;!?…{•é¸$?pB>à"1Ò?¸0õΝm?žæ·GõO?쥟Wä¥r?Ÿeã'4FGL J1708.6-4312?ƒ'2¢&¡y¿ü4 HtãØÀ9¥tæXÀ;æñ;A@'2]jÔ@N¿ö$µ?ÍI>7s3Ô?Þ8ÞîãM@YДØ@°{/Ì ?îÅ&æÖ«¿ÚWq S²…¿àºëÄØí¿ãÂ!­Ï±"¿ïVNád‰l¿ïT?‡ÕK÷OTHERunk1RXS J170848.0-431418?"7B(#²?wÜð+«?²aOæ?²¹ðs*?íckàb°?²î"È@ºÚ?´—ñ»ïŸ­?°.ål•½Q?±Ôdžä0¶?±¿7ˆi?ë2u4¥…ó?·pÖj•Å{?ºáéŒùâs?"Zì$§?Ê°'Y½'?¨©Z'÷?å÷ž
TQ?ª¨¾S"r»?¥Gý‰°dT?Lºà_œ$?º$‹ß#º7?¢~ü¿àé?ëf's?¦§1ٌŠµ4FGL J1710.9-5247¿î`{K-ƒyÀï•·UlÀ9þ¹®âÖúÀ;'óá
Ì@N0Üêù@ÞÏŒ0û?ϝ^ mÿ?ÖÔìԍ@ð¨ß‡ºt?ó?ƒ3є?ïÇ:"ÀÅ?Øá=\¬Ô4¿å0†yÇ¿í8⟜é¿ïÿú Âî'?ïÿjÿR[OTHERunk1RXS J171043.7-530019?Ø
Z[­÷?Èr¤OÂ˦?¡ìýK«žä?«Œê«ü‡?âڂýnJJ?Èèê/µàW?̛ÀgÿÔ?É~!€Æb?Çr"§p†®?ÈijÇHC¶?âüjÒIÞ_?Í÷~~µä?՟FƒÝ?¬ÈMÓLùé?Áô㮫Ó? /ï%D?à³$»æ"?®SšBÎ%?¿ÈSö3?¢´d<?Ô'yi¤Û?¹S~C†—?áó@@òí?¹AÃs<@^4FGL J1711.6-3407?ïo+A]@	"Äv£ËÀ9Ÿ6'Ú9À;$É:q@vŽôÏö"@¦NÜ%´?É;Û7ôŽ?ÉxրÂ-@¯~Þ,q@ö™ŸxÖ«?ìÚʆ¡oQ?îÝIúÑÿãÜÀ•†åb¿è`´á¼©¿é/Q/|¿á׊`@²xOTHERunkNVSS J171151-340701	?Òڎâû‹?ÀåŸ0‡U?ÆTOÛI?¿9á¯2Î*?àýµÚ:‹i?ÅWy&š¾?ÎÿìFçÓ?æ)©ì›…?ò̺óø‹?¿Éæ<P?ãÖ1Gè?Çe¯¦Ñ÷?ÏЎ)´Ü–?¨¬Ìáƒzè?ºNxO®¯?œ4~J?äÂ
kÄ?«þÔQÄ?Í뛚ß%Q?©Öäb?Åë*0_BK?®6ñ²cÿ•?ã
N0f?°" åœÎ4FGL J1712.5-4642¿å^kò'¶dÀ'^!ôGÀ9˜ð¹À;)Y•Œ@°ìaŒ@ƒxÅä?È¥©GÎ÷?Ü'q~Gƒ¢@óg†!Ñ@¢"¾"y¿×|z"«uå¿å}IÔ+¿çá~o¿é€kà£Ä@¿î""¼ÃjM¿íú¾z$OTHERsppSNR G343.0-06.0?­@R<{¸?¢	ºoš[?Êt"yÄý?ÁIÕ¼%õ?çŽò7éG?úªœ§?ºX¬…w[Ê?·	ēµË?¾SuYà‡8?ÀaëQBYš?èê{Ä¡?'l¡ð?Ä–àÞ?¢ÿõ3Øfú?Ä¢…p(?¢Õ­vxŒ€?å¦õ98ë¾?©êOÝ$§ƒ? Jíh'¬u?"'Æ1TaR?φ$d2?²as{~]í?ç6Gôl,?²s§|Üà4FGL J1713.5-3945e¿ÈÑ@"²¿¿Þ@zcÉSÀ7aÿ¨Â,À:fpÍÈu@";@1ôD?ùµ *­R´?¥#Rj†¾?°Ôñ‰o«@aw]?÷Ž²Jj‡]?ﶘ]Ywk¿åہ›v¿ÐŸv¼Ï)¿Ñ?áAxñ¿×Ś^:á¿Ô…·eOTHERSNR3FGL J1713.5-3945eRX J1713.7-3946?«eå2©ß?°eîÃ8ʇ?'ÌZ'1ù?‹\ʸ2¢a?î7h
~?²&•)œzÇ?àé-Lб?¨›¨ÉFP?¹È^­ž¯í?Á;"³K-ˆ?ë×ìàáÃ|?Áy¼!ô?¼^¿ (Çi?¥gAÈR;?ª;Ÿ?•y9 £3Ä?êÐvî‰?©"\Øé£?˜éj¸ ?ˆáٓÍvž?´-V'/'F?¤Òу?ì¹¼èn¸?¨Ðyµ
s4FGL J1714.1-3811¿ï÷&¡™1.?×5Œ	À8ÃÌõçxJÀ:ºæç*F%@"/ÊF_µÈ?ÿ %9um?»"Ci6Or?ªé^ºS+?ñ+E"ˆ¡@}:«w'‰¿£™1"́þ?ì¦a
¶ø¿Ðþ<[zû¿ÝNjܗÆ¿ß/Ÿ•\7¿ÝR€*‡¾OTHERsnrSNR G348.7+00.3?Àþ5"!#?µá¸—ó¹1?ˆ"ÐãË%?†v¬c
»?ë^h¯ÀŠ?¶ßM|»?®=	µR@ë?±w£¹á?•Œe՚'%?¥z'L)qw?íoÌ5þi?¶½nŽ»?ÅÝE	ž"6?¦(2<?±«]à÷²?šœKi–À?èSCyd°?©b7Ó¬º?¸ÜáÛÄ)ö?Ÿ /³—é?¦\BH¦\8?mÉñ%?ë~ŸŸýþ?¢1«eöè%4FGL J1714.2-2928¿æȜ\Ó¦Â@¥w–9'ÉÀ:Lp–À;"7À`­À@"ò}
—´@
ˆ~¿"À?Ìéÿb¡4î?Ù
°Â«
Û@—'YY7ª@µ2Ò:J¿ï?Wc"$?ïÿ×á¨Ññ¿ä¸¯©¦W¿âá4bÞª¿îa*ÝyBa¿ïþ]~
qôOTHERglcNGC 6304?Ǜ³é±æÂ?¹kKäÖ?ËɆà(QÙ?Â=:™iíT?ã&±M‰qÙ?Äù"âÂÖÏ?ÒmS8Ë¢?ÇÞÁ%sÆ{?ÈËs¥¦tÓ?ÂÖôã?5¹?à–y"yüú?ÉÚée·Þ×?Òéö¬| Â?¬AΖÒ?ʨœ":ã?©"3rôòË?àڂ  æ?¯ŠùáBká?Õ0+"µŸ~?«T`ây«?Ã[9‰À$?¦ž5Ð×Sh?à'Ó5)¸?¯<›ì°YF4FGL J1715.3-3832¿ïp3X¿V9¿ªl^Íë±À8ƒ~Ù#ó$À9¤*ëf@£#âqŽ@O	zÓõ?Òµf~ºC?Öa¨üãëÍ@!µÇ͉‹@G+ù4ä¿Â?$ÃÍÕ?翞æàtI¿å^*Ýúº¿èYP¤«›¿ë¡›%ŠÔ¿ïê­R´ûOTHERunk1RXS J171538.1-383531?{¨Ùï*?•d'ÏáŸE?šm§Í»Ò?¢¯×8?îõB¹qžC?¦¬´î1÷Š?—o)$̉?ñæ<
ö?¹è¯Êî?¹®ÈEàMZ?ìt½{Ø?ºe€qY›Å?·÷ÒðÏéá?š6ê•­¨?Ɯ0<Ï?¤ìª•¨?çZÕ×P?§™×d0[Â?pȼô"?bGl$Ü·?¡|­ÿ­?å"d°Ž´?îÍŌåã?§ÕòS+4FGL J1715.8-4549¿ïA£6YÀdÜ"«%³À:oÅåÀ;o§ÿê9@ZÉ!œ‡á@^ne8hý?ÓÒo##p?ç%  ß^@u‡CUÀ&?ÿgþÏSd×?ïό/MËe¿×ÛÙ°
g¿×ED'»Ü¿êE€½ªšô¿êm[}Ë¿ê…M²:zOOTHERsppSNR G343.0-06.0?…²âKwT‰?€7ˆ©aK?©Á'.¿¦?§"÷(œ'"?î
!üÿ6³?¨ã£‹¬/?ºÝ¹äÀy?·íÛNÑ&?¿²ôXï?ÀÛ»7ò?è®—J?Áõ¼5½?À0x9?›æmUcO€?Ñå[ðz,?±xçJs#b?ã3ù'¨µ?±™¶÷÷ݘ?¤´rgµ?‡…C˜S™N?É¥è7NMÌ?°èuµ›±?èK>˱=?±¢Z$,»Ë4FGL J1716.7-2808?âXv$ÁÎ@ú&€IRÀ9M'¿°"˜À;'íû½ñ@­ç"^@Ìã"y§Œ?»ÙÁÎ7?×FW}?pÙ@ªTà,%"@ÜðJUd?íay,;È-¿ßÏÔ¿	•«¿ÜYB'uê¿âÿO™›G¿î3eˆ¿ïòüÂ÷ÆOTHERglc3FGL J1716.6-2812NGC 6316?¢"O	ÊZ?™;û,¥µ?èÒê›"Ø6?¿öB"
ÿ"?ȁÑl?½¨)$}'?±E¼^¼r¢?· f«¤r?ãó)Bý
g?Í>H€£Î+?ÓÈ>bVȊ?ÉÆNS"¦?¸½áÙ/›"?£TI¢"¤á?çöÌM'#"?¯(¢œs?ÃÅÝÝ_£è?¦àdzáº?Å©}1ã.À?œ(Ç
ÅlX?ØÞ£·æ?¯]OÍüû?ÜLžeV'?­¡˜Fa4FGL J1716.8+4310?ç¦}"¼@Au¥ 8LÀ:¿,;È-+À<€g€AÙ¿@l[…íõ@¥Ÿ<pÊ?Ò Š#¯Ý~?àȶd«{@¤ò®å¨@ñ`°D
¿ìõ¶ÀÆÚ¿Ý c¸6<Ó¿äBej½ãü¿æXh¬'Ãâ¿ïÿ½OG"?ìf³ÞiW]OTHERglcNGC 6341?íG¥$QÕ?¨^]iƒ?¥'²—".?¡†_òŒ-?¦]û;K‹ø?œyªâ?êcȆ°e?Âó¹@5=?¶z%úœÊI?À
ǽB?¶g™©-²…?¬"{µå's?è@\¬6Ë?©ñ±&Ðõ?¹~ŒRî%a?1fŠcÿ?Âï¸cØ#?¢¦2)?"?ë[2:œSA?¦f"&"Ò?©Øäl.?š@gÿL?¸:&9/Ý?ŸZvÛÄ»÷4FGL J1718.0-3726¿á#îaœýý?ÄÅąU"ÝÀ7}5¨Xy>À:*ôàM/@ Œáºö·@Ϊ¦1?©šÂÓ=™?¯J+Ú#@¶w¦)ÊÕ?ûѺyãò?îÀ]ÔÏ¿Ø`Sý®(¿ÞÛ¦d-Q¿ãOl-Îo¿åGÞeü^¿ãÿíPÐÓOTHERsnr3FGL J1718.0-3726SNR G349.7+00.2?"DKëöô?ˆ-®#TTf?©¢Oì³?°ß«ÆÌ?í̝6{Pf?±%rüÐ?‹ÉߪzÆN?ÑAi%á?¨TL'A?ÂVh·Xï?êæÃnQ‹?ÂUé{Fu?³ñbgD&?—ˆK°~Ý`?±5 5?–Ïzå?ëagcÏ×? è ¥+ÆØ?ü"{7÷?{éj"¤6?Ã{­"£?¥'÷É
"?ê™0–û½a?¦ÆHøíì4FGL J1718.3-4445¿Ì'–NFÆÀ]'@.Ä9À9°"6[àÀ:áJß!c'@ …úUq!@ºizíÜè?Ñ3éܨ#?¿«ó¹J¹ã?÷rï
å?ÿ_Ñâ5iÄ¿ÒC¨ý?ï!ÿ¯"B¿ç%ƒ—×ø¿ãV;`~Dÿ¿ëÑ4Û©ßb¿ÛŽã»{ÂOTHERsppSNR G343.0-06.0?ÂLšÞ¼o?± ¿Rü'b?¼êŠk8[•?µrW^ Ÿé?çޛ‹áEq?¾"iAZ_?Äù€ˆ,Ô?º…|ðöÉ7?¤¨­zÅ?«ÔC §I=?遅p?½:OÅó¹?Çoß%»l?¤Ëðåï?¹—ðƒš?œ0#mâÅe?æñ$|¦Ó?¨Ú]'¢é?»Ä!0È?šAA· ÓÙ?±ï''Ûºb?ŸF.•?W'?êIË'b™?¤™?¦æ4FGL J1719.2-2943¿×1ï¨ç6Ó@}¿Î·ˆ˜À9Ú¨ÎÀÂÓÀ;(ÇAr'@ !f'jþÒ@¥BDH.?ÂXIؑ&.?¥Ä`A´*j?Ø»›!."þ?ö"±ší+½¿î¸G¿²2?麗*¿ÂypÚ2»ê¿æhÓ]à…ç¿êèûlˆÍ?кѢŸ|³OTHERsppSNR G356.2+04.5?Î>5ê'?¿ÍjeÆS0?°-]• ›þ?¬[†gÍ«O?æuÄÀñß?Œ©¾±?Õ9ÁõzM?ÆÄQkçþ?­ÞNù9?´3Ró?ã…:'óÂÆ?ÇxS¨v¾]?Ò1s³ÿS?­jPZg-?·H/6l?˜Wƒm´Âž?ãþCŽàŠ?¬wŒÒY¥?Ί7tÇâ?®ºÛ{´m?°äŸha.? Âî×c÷)?æ@Þ*µÁâ?±·i×bn4FGL J1719.5-3858c¿ïì;gŠ'â¿îýÕôéLÀ96^q¥^ÊÀ:‹™¯i·@€‹Ò† @Õë#Ïèá?Í:†ä‹/t?ÓÄ7Kæ@tËáëB?üû]y,畿ïÔY=ÞÝÆ?ïߘa5O¿âÀŸAú m¿êD
û¿ïú}¢Ã¿în¸å;rOTHERunkNVSS J172006-385734=?̉²m?·8dåí&G?´°2y^k°?² Uñ¬(Þ?èCWjQï?ÀV]ž‡æ>?¦ô¸ª»|õ?¨Œ>cEµ×?¾"|š-'?ºÈë$‰Á?êÀ$õ?¼ýcìðWg?»¯$1:,?—˜Ö´€O?Æ]­m¥k#?¦{	Ò"Ä?æò°o_·?©›< ¬Ž?•#YÇõ±?€K ©n?Á¡òÔË6?§ìþ'T†?ë¼µ!&?©!iéÒv4FGL J1719.7-4500¿ÒM™ƒý® ÀÃkL4"À9°üQõ–À;¥5¯v@H·"ª—C@Ók'/É?ÎÙ6´Þ?Å°"UÕJ?þ*Óé À@#T²^âd¿ËP§!íeŸ?ïüFlÊ¿è2æ§ieõ¿áȬar`Æ¿êv?A´U]¿ïՓWPOTHERsppSNR G343.0-06.0?ðe¡I?¶"Øî2©?¶vTCÙ)?² nߜ<6?è@7ÑO2—?¿
åVÿ|œ?Íúaê_?¼É8ö
j? Õ™¶E¨?¦›z±"?ç±"p¬!?¾¼•‹Å·»?·ŸDkz?«
.V3?¹è!a–?œ
]s'?å,[*¹^?¬òWÓG?αl¬úÒ»?¨Žkݛjl?´¼d¡ÃNf?™ëŠ{`Çü?å¼@ˆá"?«¾Øô˜4FGL J1720.2-4757¿Ü"jÈÏ_ÀÀÓI¾óÀ:'˜Ë=À;K§ågÎ@¤àDMâ·@¡/ÅÀi?Þ³ÞY<1?âéà¾ò·@	å'^éšc@ۚÅ都?îÁr'¿ãF¦ã.8"¿êí¦â'Q¿è"s?ã­¿î±CD"o¿ï¤rØœOTHERsppSNR G343.0-06.0?΀³´ÔÒ?À¡yâŒø?Õ}š*´?ƪ'	ªÈ?ÛBûæâ?Æ¡"Ò³Ë?ʊ!I;g¹?Ä 
ËӚ?Á+`ÓÜ® ?ÂbgÛø¡?åŸx¹úŠ?ÇcK%UY?ÔÁ£mê/(?°-ctõ¼|?ÇiwËé—?©}Ôrq?߉ ¬!D
?°'Î.wÈ?¹íO˜Ä'G?›vG—qÖ?˺<õ]Îû?»t²‡ùƒ?åÓÆϏùø?»rÛ6
"v4FGL J1720.6-3706?ƒ³(xÒÌ¿°¸XÌtã,À8§?LF)°À:1²þÅm]@>w|ŽEþ@S½Ö.u?ǚÕChài?Ø ê@%@6Vîú??ô–óT Å?énÑnòý¿Ü.®¿²‰¿á½I6ª¶ø¿èÚå>]³º¿ïÿðEwÙU?ØddIU´OTHERunk1FGL J1720.7-3707c1RXS J172051.9-371033?"=7/¥?fg/ôy?¿ÿҗء?¿!@?ë…7ù+Kn?À|Cpz…?šÑ‡Jûå? 2<êiP˜?Ä €*Ó½Ë?¿¸ÿ_8uî?êSºó8P?¿Ü7ȯê[?³ -²†‡f?–öÞ' Ë™?Ïu)€p?®ç;ý>G?宯驮÷?°_1Š;Š?dÇÜwŠœ?S¦SAr
?Æé+ãr©?¬w€PE)
?ê0í*«ðú?¬´ô-Š¡¢4FGL J1720.6-5144?݁¦~À ¹y[5°¼À:¦úX÷À<"hê¥$è@ ²šl'p‡?ý	¨ÛUüŒ?ÐŒ¢:R?ÐÜ¡'N?ÿàjْ­í?ÿøwWû>¥¿Ý¼âÉä:¿ïÿÍ?¹Ss?ïÿþøþ"¿ÂÜËG'	¿ç+ÔÏЍL¿å»¶ŸŽÑOTHERunk1RXS J172032.0-514414?çQ¸"ÙJ?À¸M¾'M?pzSF7?hKQfì?Ñü}‹3n?À–o6¤´Ã?ä2©B¬"ª?ʑ!ø—&‹?làþhêl?{yp"nÀP?×b‡¸ªèÖ?Êgc/B#?çkw«Û?©v•«úÐñ? h³æíi?ˆ+EI¥G­?Ï´%'˜48?§+U0{?é$(ƒËG?¯
õóÍþ‰?…Ï›08.²?€Ëãp…¥?Êd@ÍO÷?¯`'C'7n4FGL J1720.7-4629¿ï£='¹éÀºÆü©3kÀ9«;_QŸ/À;蚈¬â@,Z¢7øÀ@
=f?Ò&Mà]£?Ú
™¶õÊó@ýÌI?ü…jpUÊ¿àŸÖ"Ì«??ïø m]Ñl¿ë<7ž|ØC¿ïg6¥®zÒ¿ï¦J'Qž?'rs\e~OTHERsppSNR G343.0-06.0?å›k	õ?ʘc@Öx?˜òµ§™P?œfîп›?Ó9þ}r€Â?Ê!¶òRh?ÇØdMeyM?Á@AÁÕG?À>Ò17¨O?À DZÖ&ð?åú2`X·™?ÈG,ü?ÒÇ÷?õZþ?¯P›†ÁÃÛ?ÃYŒ‹æy?£]É¢'öÙ?áÅ¡_bXã?¯—(?!ܔ?Áá¸þ×?¢3 ċŸ¡?Êxktè?±#÷†Žn(?äévà0áQ?³ë}‰5£_4FGL J1721.7-4709¿î‰Gj*sÐÀºeÏg±ÀÀ:Ɨÿe¦À;œèÔjP@£©blD@¥ýfȌ?Í喝:ã×?Ò@$]Wt@,^b‹æS?þ-
gbé?åùæuë>¨?×|Š_iòã?ìÁ֙Õ(¼¿æ˱ÿÁ쟿ޒñì7Ì¿ïþŸã_¶IOTHERsppSNR G343.0-06.0?¼TÞÛå?´9µÒ.?…/Ó¿U/?¿â±¨&?ì Àq±'.?µÅ£&í?؍!Ü2þþ?Èųô2ÝÒ?…—%GÙNÕ?'¨Æ<±hø?ãc|ÇF?ȱ€Ÿ	R?Õã¹úyӚ?¬ ñ
"uÃ?¼ãêÔò«?šöž®üRÂ?áŠ&…hwÝ?¬ž
‡è?Ýýœ'O½ï?ÀÏõ AÜ?¥›hÿÕ?§Éeÿ®¥?ßNöMµ ?Á>'¢Wo4FGL J1722.6-4529¿Ùl3¼½W†À…³ž'ÔÀ9¯Ëú>õßÀ;²Lþ
@ÝS­§@ì``'çÏ?À9yþ§?ÔØVB×Àò@'j¡^‰ù@kn|Šj'?ïµïpeé¿ä±¢Íõ¿ß
J 4¨Ô¿ã‡#uP5¿ë©ÿBjß¿ïúêû‹ýOTHERspp3FGL J1722.9-4529SNR G343.0-06.0?»ò‰JÕM?­!¨§?ÜZ3…BJß?Æ{$v¿E?Ü©D˜jÿÏ?ČO!€[?È.axðB?À:
š[-?¼éû¢øšö?·åB¥æ?·?æW>sB°'?Ã3êKê¥ß?ÌS2-n
U?±©6Q=?Þ|…£KGÏ?¶ˆ8]Ø?ÓYáEý±†?®©)'¦7?Ô~3&iu(?¤%SÜvm?Ä,oŸ¬µ©? pĪ™ö†?àµÊ"à?©{¯ãÇà4FGL J1725.1-3408?øΊbð?ë2~žºÀ8ß\Q9®wÀ:I‹N};•@N.4ñ¤H@îu5¬?ÉNÚX¦Š?¸Í®ôõ‹?óü8Dêëœ?ü§5Ù«­m?ãØ'>2j¶¿Ú»k{y"¿çRª&¯—2¿åjþ¦Ž ¿ì¶ ¸Ý,¿Ø/EâOTHERunkNVSS J172445-341032?z!ž×ʶ?p¦È«ŽÜ$?†!›û?‰ÏåWÿŽ?ïs^RdZ?ŽweÞM%L?«Ø
³«Žª?©;€®m—?£Ô¾æçÓ6?ª2"'ŒH?í36VÉã?³5gwÀX€?¼€Îö|þ~?œ
¿é¢?ºŠO•Í?žAď¾?éœ.Æ?¤Gÿ%â]? è
[ÿ6?‰°RR&?œYö<ˆ ü?"»Í>Ü5?îÍEû?'xœFQ›ê4FGL J1726.0-2843?îÝ(Έí@
çTm?žÀ9ö·ü[/ÑÀ;Mx2@Äì@ Óc®ün@7‹7GN?Åa°ÊÓù?…³sy8>û?ÆZgª‰+?ü{Ã	ÕkØ?ïNj׆¿âÁž€‰'\¿ç	ýڶſåf:âT¿Ö¯šâÄÜ¿ãyÔ½\OTHERspp3FGL J1725.1-2832SNR G358.0+03.8?Ê·BtÓ6?À'ƒÈœÈ?ig;—ã<?gë8'J?éFªó˾O?À03W'£M?ÔjðE/*?Æ@2œG-?Žr*2¾&Ç?˜—É8[ž^?åP¿4¦oÏ?ÆD€V
Œ·?Ö>ÂÉ̾`?®ä‹«çp°?§íQwÕ©?‹!,'ëã?ãaɃ¨³u?®*Ó@][?ÒWÀ˜,&y?®'oÕÒx??±ËÒ¥t?'hÕºã?æW 캢.?¯¿Ä&Dß4FGL J1727.0-3835¿Þý6¡~¿ÿóÐFÕÀ9á¿uÌ4÷À;ác\ƪ@ëE	¬§@a/	ØÆÖ?ØY<k?éÇE8ï4×@
ÜT^üå™@'Ö†ßÙ¿ÂXG"©¿Ùn<‰J"¿åî'Z·Ü{¿î‰¢«'¿Ô×Q?ãšÅ¿ïÿs³VBOTHERsppSNR G350.0-02.0?µ±UG˜uå?´¥eó¨?†‹&]é§W?:åz4,q?ì悔•J§?µEIÇÍN?ÒÂE$Wš?ǯÜvI"?"|­—•®?¡Û?Vw®¼?æaˆgÀ?ÇJz)ÒìD?Ô¨§ýf»
?®Aƒ@­û?Ã-ÀoH?¨D°×¨"?àêà'Hƨ?°K†^¹/?ÑôÔê‹?Áb&Ú	²'?ƒÝµÀÑ®+?€avgQ†?æ¶HbD?Áó¤e£åq4FGL J1727.6-3050¿Ñmk£g"Ï@@€"ÐÀ9¼'xêÍiÀ;<Zݜ'é@/§x#@ŸìÝ
Œ°?Ç~÷?×q,½ùf@	C¦GýÆ@kóā¿ï·âÅ\–?ïøÙ?Ìɝ¿ÄðÂuZõð¿åZOÈl–¿ê} >ÏH¨¿æû¼Ú'.OTHERglcTerzan 2? ?ŵšr?"(ë$Ð?Ö46ðÏ?»ݖ&
G?ê{ט£?½Áõ7KtC?¸ß[¹ž´+?°t«š#?k?ÒHHg ¹¥?ÆÊÁY†LÏ?ã¿ðU;̧?Ç&·t0•D?ÃW·#Ùf!? ¬A¼èb?ÈÅ-ö+p?¨jMHw°d?äøƹ~åœ?¬,eȌ¼?Á@äu‹?žáAR9ô|?Èêr(÷?­—¿Og!<?åu*X•U?°ÇdQÄ4FGL J1728.0-4606¿ØŒ5˜hA2À
çO/<À97cf×¥nÀ;-±@óL/Çn@¿Ue""?¶¯ÀøXA?Ò>¨\U†@"q VL=?ø3
ÎʨÛ?ïÿÙ¿y}¿ß$Ěúݿ჆g­Ó¿æ¥ÒWPHî¿î¸Ÿƒ¾f¿ï÷q†U7OTHERspp3FGL J1728.0-4606SNR G343.0-06.0?ªð—HíI??£qeñé¢2?УIöÀÆñ?ÃNTS!ó?åÿQÇô?Ö̬î4?¡ ÁOQ&?£»û¿;Þý?äÿ'Õ?Ê
†'>85?ÓÜÄÜÓþ2?ÉQU·¢†L?¹p›"·<
?¡LCPC?ã\U¬ =t?´ŠÃ9À44?Òë-Á'¶?±h½À†Èª?¥wp0¬hà?'åö,ur]?ẛ‰,C°?²Ü¶ ‹–?ÙÛÚç'ë†?²ª…—\"4FGL J1729.2-3641c?ï
}¾"¿ôŸ(NÓ£À8Q•p?-<À:LÁ¬Zg@·
Rê2¹@ríãÉª?¿z—˹&}?Àp£$è@SÍÅ@Ñwò)þ?ïà!sNÑ¿áˆ8õë¿ákz¢]z¿éOJ@ì¿âŒÍ}÷§—¿ë	—"ÆÔeOTHERunk1FGL J1729.1-3641cNVSS J172917-364008$?ÎIÑ5çÌÏ?½,6[mlJ?· g
ûH8?¶‹ñewŸ?å‰~ÐÆ£Å?Ä~Eçß?´åžÀs…~?±ÔIÜv?¶£ ¿jŒp?¼n¿Ñ?êŽØ=Ã?¿!Î:[?Á
s­ÚJ?¢Ñì€Q?¿å'µsO?§Üۈ—‰?çÀ°Åæ'#?­Ì\wî¬?§Š4Zp?Œ§ªàÿ"G?²×—®K R?™{?f•ï?ì34fðê?J¼é%Aì4FGL J1729.9-2403¿äßÖâá@@]•ÝLwÀ9s†öÿ¦À;)½¥œà@̏›"ï·@ìB 6m?È{™=´?â}
!P² @"‰|ëãé?þéÁ¢w8Ç?ïü×÷£:,¿ÔÌÕUc¿ã¤¡Ý5¿ëÿ‰b"ʨ¿ïõê28ap¿ïù)¢ßÇOTHERunk3FGL J1729.7-24081RXS J173013.1-240234?«žŽ+FÄ?°¸¡'Ðøÿ?ßèkQÜ=S?Êç™n|Y?Ü£Âê¾YÕ?ÉeÍ
Áyž?¦%yqJÜ?²/Oþ4\?ãú‰ÑóŠ×?Ì%½†?ÕFJ,êÀö?Ê`ë3èÂå?µ›Ò"´¨?˜dè؀?àò½EnŸ5?³‡ÍvùZ?سÁ€šm?±>'xË7?ˆRÎÃ.…?møÏÚ­.h?Û6­;06?²zÜcˆÖ?ânU¯'?²šï'æã4FGL J1730.1-3422¿Ë£ë+²‹¿ÂGUêmFªÀ8¦Žt¢À9šÍÔ3É[@¡Ìzd@½Ofo ¢?ÍØ&ݏg¼?Õëòa±ËÀ@'؈v\?ö¨Z†¬Ø¿Ü«®¤Ã™G?ﬥDȆí¿åހ¾×@Ä¿éclK'µR¿íT¿	•ªø?"Ö9`°*OTHERunkNVSS J173013-342115?a}ò¢ˆ?e{âz ?qÑyadü+?}÷ÉíF?ïÊß›$?…!³·¤Ô—?—è"؆v'?§¯gûb?Öµ1geæ?È_üt"Ì?ãæ&5ˆØþ?È!tp+¨D?³cNbDÌ/?î¼¨ÂWë?ÇQ+3—ãp?ªE…&­æ5?ç¿KfÑmŸ?¬dÿ&ÁÎr?iù`Ahk?Zœ0Aäö?ÅA(P¹/?²\Õ¼1®þ?ꕼ‹SŠ?²†%e<4FGL J1731.2-3234¿îdz§'?å$Ðd1À8yÃ
0j+À:?–fß2*@`¿ÞQÚ@,€"Þ?¿^•–Ö?ÓhOŸ¥wH@»4¾?ù@w?ïÂ*|«LJ¿Ö"¦%=d¿àã7r]¿ãÕ¡Qô¿Z¿íoJpfši¿ïÿ¸aÛ½+OTHERspp2FGL J1731.6-3234cSNR G355.4+00.7?'ÜÎë(¤?wFuðâ?ÔkŽ+Â?Åï¼Yth?å~Å®rXc?Åû>¨cr?‰W‡vïr?'òðWO}?Èù(Å,?À¦à?é˜ã—ó¼?Àã¢îÝë?¤é™ûl~?ˆùÈ%¡ÚÜ?ß
ªÍ?·ÉY@€?ÞUµÅ[0?¶ÊÅçV¤‡?i[½³y|]?Xç‡]{—?řÖìÞ%?°¡3w¼ž?ê€.‡ýD?°Ö
Ž4FGL J1731.7-3445¿²Û\ª_kt¿ãØJ¯P»À9£££Þ–úÀ:ÍÛÌDÑ@!ö]¥øw @mŸ¸—Œ?ÂxžözÆ¿¦ÉÍÂÐ?é÷3]z"@û»!ԑ?¢·µ8†">?è–._äÂ¿è‰ù¥ôò¿ß''%οêNûæ•Ë¯¿†WýS8OTHERsppSNR G353.6-00.7?©A›Ô§{?¤;j(³Ì?‡®ñq¤êè?'ó<fs¿º?î
*|îûœ?¦çèºÞ¯?±ñ¥«¤`â?´Qm"S‡Õ?‡Õʐ쩟?˜uz¨.Ò|?íbt GÁ>?µ\
î:i?ÈÙ®º:Xö?§:­ÞvÙG?±vŸC#¼#?"cؑ(Zv?çšÀiò>?¨§ùdÐ?ºXJëXÞ?¡òêpV?"–±r
é?‰\ƒ©o?ìH«,?£³r:²n 4FGL J1732.8-3725?ì¯;íAŽÀCÁð`À9eV2;¼oÀ:ìÍ҆J1@"~'¶Ñ@åH©¼ýL?ÑSÇ'q^?ÏmŽä3ñŸ@ˆÚ¶š[@?¯uxýî¿í$Ò°+¬?ïõ9Ó`dÅ¿èê$@ÒA¿ä—™^á6ç¿éÿD^(Õ6¿çÃlfZ§ìOTHERunk1RXS J173250.4-372144	?ÐVf½ì³?¾|ß\(ØN?È·kÕ?½d>Úüh¾?áӞƱC±?Å%I¨'?ÁúÙðB?»«ÍÕA|{?½B¥v^¼î?½*Ø5Žß?çÙ%š¸$Ò?ª
<œ•?Ä3¾p/.™?¡sfi&sk?Â÷§'i)i?£UL‹s"b?æ5&šéÿ?©u庲ۉ?ŝéÌá˜,?£4¾¼—žª?Âþ;¤4'å?­‰ø.6•£?åØö£ºý?°>¢ 1ý/4FGL J1733.7-4734¿ì )ZHÙÀ@š$À9ô§5jEÀ<Tsõ›@ ÂÄT­×@ÔF=Ñó?´Ÿ&y¿°ÒÖ|#'@Òß5…@h]‡º;?ïûw¾Q4¿àÝe4Ù&¿ë¢=aàDÏ¿¬ø[EöÚ<¿Úìé7fž›¿Ýã_ ÏmçOTHERsnrSNR G343.0-06.0?äŵäT|?Ä.Yb^s?}Ô]"ó*?v_Å`ÀL-?ÕýBÂË4`?Ä
Òìå!?âøÀã?Éþ´ý,%L?l=zë‹?@ªâß1Â?Ù×ÚEÀ?É·ä¯ûW[?é#‹Ðk
3?¨ïÅeÚ3³?'Â=LºÑ?}æ5Û4˜?É9‰Ð_ß?§;¶› $?éhщè?«[¨<N°?•	'Ÿ¾îï?‡‹ó}£_ ?ǾƇ½úƒ?«&Ð¥<Zb4FGL J1735.7-3026?ëJ
iø ?ðZ|MXxgÀ9êCÖ¦À;Ô#£s7/@Ã՟.Y@âñíÅï?ȃ§¿Í
?ïÿ¼¾ŒÃ@ÖþqŠ†×?ö39=cc¿ïø⚔k¿ï|˜6Ã
¬?ïÿ÷fÔJp¿ßhóžó ¡¿îÈ3'˜¿ïÿyýò߆OTHERglcTerzan 1?'ŠPç·?™¤…i"?ê`'‹Ç?ŹIxéöï?ÄN{˜îìÛ?Äöd ;Œ?€×?1"í?'lΛËr*?æ܀ü:?΀ˆÙ!"k?Ó?ä?ÎFz&øL1?´YHL³?›ËSpb?æQ½|Š>?¯aæEo;?Ì­]‡°²?«Äؽ€V?\ºú"AÂð?Y–mŸ«p?íjº/=ƒ?¯ïh{U ?´7B™-×?¯_`
b
4FGL J1735.9-3342¿ï´<*'Æÿè¼Ý W
ƒÀ:I¡òYNÀ;•ð	÷y@$>ìW¬@?öúReŽÐ?Òõº+àY?¿/øìˆ?昏Bþ'Q@L¨–a«Â¿ÙÝ>‰þq?ìÕ¨]ס'¿ë¶y¿¾ë¿àt¹°V$¿ÚC©blD?¹kt~hLOTHERsppSNR G354.8-00.8?À46­$ñ?¼dõ©=T.?[8'ù²æ?U£©ú|<Ý?ëåV:BF?¼ƒ*aV?³Š¾b''?¹è¹ÄH?|…ãözӏ?"£êLÿu?íUœkÂØ&?ºnØÎÏ;?،‹N:}ˆ?±IfŸ'?¤uRÐÏ?‰W©%žY?âre+áDM?°Õü¦?Ç%;ó?³ïÀÊä
"?‡ÍÀcט?Ž'Æã•ê?éÞ¿»»sÁ?µ×LHÎrÕ4FGL J1736.1-2628?áÛ6:	ø@Ž)#øÁÀ9Ë~>Ê@+À;!ë¾íç@8Å]F­@"¨~8ë?Ò.!%"?ގÍbÉÎÁ@z?|ÑÔ?ø@ƹã;#¿ïýV½{öñ?ïþ¤ ³¿5¿è3«=°å'¿æÌü¿ïù÷<âß^¿ïö.$ÖyOTHERunk1RXS J173614.4-262806?Ö¯@«|X?Ä||µ¾I?ÈD3?ü2›?Â;L­Q0|?Ý.¥´…åZ?ÈIce8ÇF?³¼ôÞ¿"?¸9I7]Z?àJÊë†ø–?͹æ[‰5×?Ú©ºëº^ð?Ëø÷›k?Äï¦Ì¸Õ¦?¡'CëÞu?Ê Ljk	?«ˆ ÆI¦?ä27	Ô?°sa`¤f?®åFÝ÷¢ª?'Lðdu×?Öò{‱Â?¶f¾7n¹D?â˜m à,õ?¶lâÞ4FGL J1736.2-4443?ïÿtŽaÀç"~§¥ÌÀ8¶A+Cz©À;›<Õsd|@4ê³èzR@.Oü—•³?®éùOÛ¤?×{z«í¯@%	¼râv@n¦R9³«?ïóÝ£C<¿³3ãu!¿Ü<Î<Ž{®¿åp³[â~æ¿ï ‰bi׊¿ïõ8%á;OTHERglc3FGL J1736.2-4444NGC 6388?©­"͂9©?©â?ã?èâÆÁ

®?Ã×ØÐ+Ùå?Æ	œHw:ß?À8QÁ4t?Œž½5ٔ?·¬~½ô·?꯶Ml«?¿]Ñ­h|Ø?Ãw:ø©öW?¾°Ìå2š™?¤N°rý²ø?™­ÉEâ?ëÈóç œ?¢ˆPLêV¹?·'Žp!©?ž	õå5¨n?'ý~±µ¨?{
g…K`é?êf&"pK?§ÕùPéWD?Ä'&?°!?¦‹Õ>Þ$n4FGL J1736.4-4052¿ï«îÔ<5nÀÔÖ¡aä÷À:PfiÁdºÀ;¿ÎçY@@XÍq7zÁ@²£Üºî?ÈPG@0q¸?·ÀÙú]?ò4Íg&Ç?þ"š™ÉÀ¿à,ƒì‰*·¿âò2ý®A¿íå*ýÌ=?Ó©£Ò؈¿åàÝPþu¿æ!μ'gOTHERunk1RXS J173638.5-405203?ÒÈ=õ·z¼?Ã¥îé;?ƒ·óž§':?êÔï9t3?æM6©¤™?Ð/>¥?àÚY8 š(?Ê47«Õ_?pCÉ6[j?…ÿ2¥ÙR?Þ
AO™òC?Êž€M?áS<[X" ?±qHñȪ?¢9xý4KØ?†Kälï?R?ÛX)¨nE?°­ÑÇÇi'?ç:ÿ·éa?·äÁJ "?'Ú+ä²?QÂZZ?Ð^-Oë†?¸ñ§Áé{4FGL J1737.5-0313¿éitäÖ@-§C"º"À:{i³"ÜÀ<7dè·äÞ@ÆUhgG@üó:õŸT?ˬñ»ÅI?âʹaµý}@žŸj"ò'@
Þ4(Q¿æ²®¨õW0?ïȳBb%9¿Ï_Qߛ±w¿éQß@lך¿ïÿY¢Ò1¿ê8PV×OTHERglcNGC 6402?Éjnëß©U?¾tjéˆø?å:ûQEM?Åñ
|ýÄ?Á©£ÍßAt?ºß«ô_nF?ÓÌ?ͺ<O?ÈqÃŋvå?â	d¦R¶¯?'¾·k%?ÀAíË@¬£?´o}
F?Î-œrŒ9?²Á4"iÒ?áPÂ)}?¹ì´#??Ë] uç}†?ª2 ºœ?ÕµKl<ö?­1ËÎ]GØ?ÚQ×^QX?³àW¦³?ШsVB³²?ª1ƒ}4FGL J1739.6-3155?ËžP|^¿Þp"ýþs
À8¤nM]À:X"@pǎŸj"@	:ß.Ï d@_å Ù(ü?×6þ™Îs@´ebZh+?ÿ
¢ÕØd?ܪ(][Œ¿åAxÀÛý¿ènrÚ/­¿ì,` ÿ"u¿ä}C!½¿ê¿ä§Œ¡c'wOTHERsppSNR G356.3-00.3?·zæ´µ?¶iÞÅfh?À/_оJ?ž¿ÄÀª`?é—Q{ï–?ÉMc^Ð?¶¼>p Åí?ÁE×­ÍoÁ?¿‡p?(?ÅZ†‰
5U?é6gCä=?È}ƒƒ,ÊY?º¡ÄæS'·?™†üŠc?Æ9CØ
ø?¯í?¢öh?çvm2Ý
?±¶Ïߋ:?ºl°Ní­?Àèíªå"?•9 ºÑM?±ôr(?ìœðe·Ý?ÂU_pýÝ4FGL J1740.3-3058c?ì}¿¹=ù¶¿ºÒ¥ÿ®vuÀ7ès¥ê
À9¥€!ùO@š.êÏ@E×_ÍÅñ?Ǿ%ÀÕ?ДΣç{O@çžóu®?ó»›~ñ"?ì.¿eÛüë¿ÓƼýÌÉó¿æT%B|¿èm`öºÜà¿éÆ&Tþ_¿áº­EH­OTHERsnr3FGL J1741.1-3053MSH 17-390?sö*,p·?u¹N­M¶Œ?£¬êâ@<!?¯>.@ãý?îDýµ£]?°ü´HF?5Ýgôj?'Aô"ïôÆ?Ðyà¼?ˆô?Ú×À¸6?çF¶Êj›µ?ÃSéMÆb?­ ôì•ô+?ùšüð"È?ÄSŠC^ÿ©?§âv:b?é ^àÓ?©¢ï£ͺ?Uµ°?ýb?Dâ…ZªË?…©ªxÀ?¦š+ï"@L?ëSºãÁÑ?¦¨OµE:4FGL J1741.1-5341?Üü«\d¯ØÀ(¨"1¡À:1ôú€5À;¼K±¯:@n¢ÔUØ$@t£%3–0?ʏ`Fþ?Ä(©båR?ø'›k*ñE@MGva0G¿ÑßrV^±f¿éQK·Žw'¿ä€–ÉÁ0¿ç||Šiü¿í^æ¤h¿ïþÞ&'dOTHERglcNGC 6397?낟U"U¢?³J3gzaé?¢"!Þrë?›"‰ˆ;?º¡td#Ýj?¯ä[…ËW?í´íŠ§ƒ?¬¡HeX‰?"e"3@'?ŠŠ'ÄêÇ=?¯—ÆH¿á?ª6ô>ì?ç¬jD?¬UÝH?«zØõç S?"lƾk'ƒ?ÊpérhŽÛ?¨®–)á?æi±kü?¨üÛmè? ùê˜øz?†Ô"o%a?ÑÇïJ´%y?§c,Zu±p4FGL J1741.4-3046c?ïrÎ0±+¿Éú³åË zÀ9MÛ:MÙ¨À:ØZ@ä@[¸b‡Š@Q¬šþ?Ò±–¡]³?èzÎg×®@à‰ï•O?ÿ³'ú;ñ?͇…oëö¿àZ[–(Ì?×4AðeX¿å"†bZ=8¿ê'Ì®š¿ïÿôým~‰OTHERunk3FGL J1741.1-3053NVSS J174122-3047120?}`1þÁ?ˆÈ壛^å?È5ÔȦâe?Ã&³åDx?énŸÌFSi?Ãawš×ª²?™OÜ
ؤ}?˜¬õ²í4?Çu+4jq?ÄÆk0–Ê?éX6R¤ @?Ä!ž÷¤t?µ§êÞËÍ?"VìÄ^?Õk¶	`
?´+®O¾•ƒ?â•'Ÿ˜V[?³¸öŸ:ÿ?¼FY T[?w=$pb ­?ÊÍÅâ©vò?¸ÂüUM:0?è͝mï ò?¹*S?û4FGL J1744.5-2612¿âñH"K@?ú«‰†&À9
	A}À:Óeµf~º@©Wn¦Ñ»@'û'½?Á}Žá"¿Ã?¸?YV†J?ù•œdO4ñ@2¯Õ›'Ž¿¶̶Q‹8?ïãšn«¯¿æ÷?ö:.¿åµŽÚù¶¿äÁN·8¿ÜžWn{ޞOTHERunk1RXS J174419.9-261230?Æ:RÅÀ°?·q&mQf?¦jGs,‡?­NWBHå?é
Æ×]Ì?¼P£¤ï©‰?Ö3¢.'?Çb'-ùJÜ?¥Ä6çS°?¬íšûñÎê?ã‰íå‰Á¹?Æõn)×Â?Óa–Ž
Ž?°ê͘ßÓe?³ðK«¸ý?œQ¿¡Zÿ´?ãÑ+IÁùš?°ïwÝ_Ë?Ò^¦$xå?ª«äpE†=?§ª¥z<÷?ŽW‰£?åV–YϾ?«)å˜Í{4FGL J1745.6-2859¿Îqˆ\Ê7¿£ï›ƒÔ‹]À5–åápÈÀÀ8ïlÒÐ@ "_§ÛPÉ@…+%G¸%?˜…ö¤Œ'É?ÅÄ¿b+]@/
'Ä"Bh?î•‹Â|£¿ÀÎÊ}è
E¿Ú@ "®¿à&cvÇÝz¿åßEuU¿é<ëج¿äç›O|?OTHERspp3FGL J1745.6-2859cGalactic Centre?¦Yv9½™?ÅÂË»«ÊÝ?ÖJ¶çï¦?ÍÍ:pXÝ(?ãrÍ(lT?Ïçmôö?p6¬Õ–?†Œy¨Q¨ñ?ê[h6Öè®?ŗ²O/?Æ©½ü\T?Å'7¬¹Å?«
}dïaÙ?˜%PŽVÚê?Ðr=‡üª?³Lð±?æ9e²ú?³¿¥wvÖÚ>­w˜ê²±>®êéTr'í?çéÛs‹?ºV1ýÚÊ?Ð,Ekё?ºQv=‰—4FGL J1745.7-2506¿ï¤»=O¹?ÿn$…ñF)À:,]VlÀ;À9'ÈÅ@'9òj@yÁ­?ÔöíM"‡?'xë¤@ä5À¬-?úϽ<¶ê¿ïþ~üà;?ïý±Ü†~4¿ÆÐîÚ雿ê¸1Ûã@¿ëð`"=µ¿ðOTHERunk1RXS J174535.1-250440?¶`~¾ŒëŠ?¯Õà®v?ßÿÛ৿Ø?ËPî
d ?ÚhoµG?ɾ®ÔÁ҄?œe1Ç"8?§ÜÔ¸»m­?æ4ëgì?Ì"—ÿýL?ÒCÁÎä?Êçn†'þ?Äâq`'aT?¡ûpÖ²ç"?ت*ž‡>?²SÛÄ1s´?݆%MÈ?°ê
—z¨?Ž\4Ìkx6?~]û$N7x?ê©¥%›ˆ?±³Ô½$"ô?Æ–¢Ú^?°åƒÏ&—"4FGL J1746.2-3342c¿ál×m©jŒÀºAå}»À9¬.þñGÀ;ÑÙ|¸@ôÔ$"ï"@Çz³$…?Ð졾×Ñ?¬Mîd;Í?ç+8ÞøÅ@JÏz?ï~E뜛­?˜¢"ŠwE¿ê)æž/*¿äDïž3h¿Ý
Š2‰~¿ßÃ	Õk׿OTHERsppSNR G355.9-02.5!?²o¾"®Ù·?«	ýŸJ?qÛ
Bì[?j­¦µ{?íèwUžð?«œ¢z¢a?Ԉó%v?š^.î¼Ã?||Šú|¦&?Še(´Õß?傍^xƒx?ÂDÞ:㒃?ÒP]c—?­µ[½É?¬Sº­¾H?*Ë4íB?啬ô›Ð?­bÝ.~?ØwÙ.nj7?¯-r_ÎË?5©Á}<?rqK%V!?ã<ÄmÄï?¯&úyµü4FGL J1746.4-2852?ŠùÌ=¿½¯+ÀçÖÀ7b·«cÀ9¨ä:§›»@ €$±0d@­ÿYçÒã?¹²Dxªâ?æGa=‡Ÿò@'¡"¬S±?ÿò©ëJ¿ïÿÖ_Æ	?ïÿu–…#¿É"£{Ѹ¿á͚ݼ^@¿ì–à­F¿ëÿfèle"OTHERpwn3FGL J1746.3-2851cPWN G0.13-0.11?š‰ÌÝ®ÙA?»ömŽ;?îÀ%Œž´2?¼aßâÝÜ?ŠãõA6?™AaÊhH|?h3ùEŒý—?t—æ<–'#?ëÓ¬b³š?¿£
ð¼4?ÀRÙi^ý§?¿wu϶ ?˜¢:³?‰ð§ó?çGZÂÜ`P?²¾îvø?ÏÎBóÇ(`?²tÚ4֜>ápu7Üø¡>Ú{".Ï~?íu²Ë…ŸÂ?§AIl7?´QÞ )C?§èØ$B@4FGL J1748.0-2446¿èg£Ho?û&òIÀ7C¼¾aÐÀ:ˆ?›÷Aë@H@
²@ú¦Kaþ?¢ô2ÂJò?Ö'½3Q¼@0¹:>À/0?ú¢3'ÒÑ?î°Ý$•¿Ñp*
ag¿Ýù˜kñk¿ä¸–IƒÑ¿í_›¦º¿ëVxHOTHERglc3FGL J1748.0-2447Terzan 5?V÷‹"Ò'E?R•±_JÀ?ì"¥f$?ºCfM?»ðԁ†A?¹ó •œÏ?duÜ|¸	?q¹"¬6ý?ì.qº¹ýC?¾ä¼¦?½èÉcL0-?½åaø¸ìt?€+™@o¿C?eÿJáÚË?íeÀLÝ@4?–%Ÿ´ñþM?²ÌŠqw?•@j‡ñ#n>ûU{·'u°>ö
˜çÙÛ?ì~yL²\å?¤ìrû.N+?¼
€B± ´?¤ëÖô¹?b4FGL J1748.9-2021?½jy4@Ç@X䓒ïÀ8íÿS1Ö<À:ä	EùßU@§ïŠçÐ@¤ê/´?¸(^ÿûßp?Ò—=í§@=Ÿ¿MˆI@Åì•j
?΀%)ZAj¿ªnSà&ò¿àê:†ä‹¿çt7ª'8¢¿ê_gJ¹¿ê¼2€…Ì]OTHERglc3FGL J1748.9-2021NGC 6440?'š¢;7}È?'"ñՊV?ä=ŒÏ"6?ěd‡ò?ÕÅÚ®C¸?ÄAìʪ|v?¤6lGâ?©§º´êMÙ?àÚÑzÃv?Ë'mc¼Ì?Û¸V<ð3¹?ɹËÏ]ۍ?·ˆ"'¸Ú?›zFãÀžÿ?Ü«éáCÌ?µy•èö¶Ã?Ýqõ°—þ?³ƒoEaؗ?£pàA½?'šÈq•n-?ЋƒW£7?ªŒÓÁßÛ¶?æƒn½òúI?«c
"4FGL J1749.5-2747?ÁôÀ9t'¿Â1²ªŒ°þÀ9yòìòBÀ;gÝkí@Õ±šl(@mZ˜?тl¡"ãø?ïÚø4H‡@~x?'æ?ô‡×¾˜?ï5ø_w´Â¿Ó'óÂÚۃ?åDª¿[Ë¿âÕub'¬¿ì/bCA¿ïþŒ}QdwOTHERsnrSNR G001.4-00.1?z"d­?»ma
D¯?Ë^l
Ô?łRvá0i?èô0½'2x?Å¡'(þ ?…ÃÉiä?—ò\Î[?árð¹Œ?Ñr'¤1ô?Ý8ûԀÇ?Ñ@Œ«)z8?°tJnk‰?'Ði×D#?ßñ…'?·8Eú½,?Üáà‡ŸKŒ?¶ÖX—}??^K j‰jü?S5Ñ¿63î?ê]¯åh€Õ?º*7QÞ¦™?ÆLª)ˆéÔ?¹üw¾T$
4FGL J1750.3-3702¿¾!ÈoÎw¥Àäõ8À8êõÚPÀ;RՔ«@&¦ßh±@'~D©}<?³éçdӔ<?ÑçäÀ´e£@AkÛm@ÚԏŽÓÃ?ïÿ6A­?ÍÝ%OšÈ¿ã
œ5ULc¿ç4"䤿ë68Öá"Å¿åȊ³LÉOTHERglc3FGL J1750.2-3704NGC 6441?œÁ¦‡cü?'EÇ@‡W?ßѯµ]'?Ä×oaö˜k?Þb5麣?Äw¨ûm~?Ÿßæs$¸?¡ìu&{?åˆa¬¹O?Ç䎦'ùw?Òö?Ì?[?Ç!ÈKqÖ§?°ÈbtLJ>?~Q±	'½?åìMçŸ8™?²÷cÙ»'?Ïê—'\øy?®¶×[dŽ0?®h¬tÀ$?‰ó)ÎZò?ß¼PT,2­?´´Á«v
4?ÜvöE5N?´êžIt¦¼4FGL J1750.4-3023?Ú-Ѩøî¿ú'Ã^À9÷q'ÒüÀ;hšQO}í@º†è¼í@Q~B%>~?ÒËUhè æ?寡]³9~@lğá§?þxqƒzô=?¬Ç‰£'Q?á¶úc
¿¿òØ`eÇ¿è¦Æ¨Æ]G¿ë7V]Ú¦ª¿ïïwAU	óOTHERunk1RXS J175019.0-302654?‰Ràù/?~_
á[?®³·îåùv?«¤›³o?í°¨Æ…?¬ÌMø¤öù?°øÅgn:j?ªsJ2÷ų?¼:/Vêìþ?¹`êÖ+´?êY¡h4Û?»'êñ?ÀdôUX(?š..qɬX?Å\ÒHü?¢šC% F?æ¢rBä·?©1[AÐ?¸`Èa+õ?˜8SôÞçÎ?ÐNˆ="£?±Ão÷ˆ*r?äÌ¢Õ/Ÿ?´)Åè%Ï4FGL J1750.8-3106?ê¬>	Ù{:ÀÊ÷?gÀ:h²qôÀ;®†Ô@o|—@V[~«×Š?ÓTo—4?ìϵIùHV@©ôafLe@Ù –¦¿æE"~°	H?ï‹ÈUnÇ^¿Xøš$W"¿åÇ-»úír¿îÁÛ!yLr¿Ú–Ý&·#îOTHERunk1RXS J175042.7-310312?‰Ï>Vp7Y?"zó|Š?Ë;—Ö?aB?Á¨Ôì/€(?èÉÝfÑ?ÁùdÌ_#{?§œ±âpAC?«#äsõ?ם!ayÕ?ÊOÙ2šÙ¥?â·¤1z?ɜtÈBë?À3-²m'?žtÇuÚ¾g?Ú?}JÞÊg?¶@׬ÕB?ݦì0ÇþØ?³Â1€kp?µ;(Ýńí?˜¸û£c?âöx`ù›?·¼ëèÇë?ÔÄEÌ«'?µÌ¶ã"5È4FGL J1753.2-2848?â9Ž<_¿õ¶2ŒDFÀ:^ıuXÀ;RU.‹.@'Ê'š¤‡@8Ã`<€º?×íK<¿N	?賁6ÌDè@
*=DŸ@‹¤íµ¥"?ì€BŠ3ö¿ç)BïhÙ¿Ó•j \×F¿ã«LŸjéÙ¿ïÿ»×²¿ÜŽÂÛ²BÞOTHERunk1RXS J175328.7-285014?—u{ÕMš?"…™|LP?Ái•@¥?½ŠÜº8?êêû¼j?¾ åd{]Ü?µ=°‰(wœ?²¼yoER?³üfù«\
?´ñG?å´?êؽ¥…‹?¸‡"!š?ÄᣠϪb?¡!¥¨CŠq?ÉÞ˜?¦×3Ûv¥?äPY.d?ª Ê%ْþ?ªi9Bv±_?‹›@)™('?ÇûѲ›?²EzG¬?èZx*,C?²müB7A4FGL J1754.4-2649¿îCL®.|¿ãåjR"À8ôç¸5fÀ:R¦'¦`Q@T\>D^T@(obŽj'?ÊÉÓH<ç?À˜|¹)?ü}[
Ѻ?ö­…¼?ïÿ%¿Ø·¿æo—@G¿æQî¿æµV¿ç¦üX«'À¿ä'/ÿÌÿM¿æQµ4)Ó8OTHERunk1RXS J175501.7-264954?šQcߙT?–ä?öWÒ?v÷˜LCc?{)¥·–·?ï6D¨j¯?š_!;êò?¦íŠ§_3?¨=©Þò‡ä?_îÕ*…x?¥b
Ïq~?í¦'èL5á?¯Àí.€£?¿ný½õ‰?¡fÂ×ç¥ì?³ü6$Äø?˜™ÝF¥OG?钟Á—ȯ?¤~àP½Èd?…N¨]¨2Y?qpÝ ´?–²¶þZYX?'íÿ†[é?îõ/¦–Œm?†bv3
^–4FGL J1755.4-2552¿êkHJëX¿Ól†á­¯À8>¡%À:"Où<—`@ ,&dä@ÙYæ%cg?Ç2>@­o9?¼Êm!¤W?þKZ;µ¸´@Û´¡ö?ïø׊•ñ¿ÚN`ÐTí¿è#¿dTh¿åÞ$ÿ¿éó`µL~¿Þ¤pMOTHERsnrSNR G003.7-00.2?•ŽK9"F?'®B¸ùLÐ?˜ÛhöĖz? Ê¡ì1–'?Uð*?¤ãû"«?¬ôµ¨C?«/?…©-)?'.EÛªÔ?—bÅþ°\?íŸBxôð¸?®ÂÒáfAð?ʌ­Šìt@?¬%;<Hà¡?²
˜»JwV?™'¾©•Þ*?灅Û"?­å§iñ,'?¡ ïû
žF?‹Ú7‰p/?'Uìã'ÁH?z­1é­¨'?î[A™3@?}0L?~¦4FGL J1756.1-2516¿×FHj8>F¿À;÷ÒßáÀ8U®mf4èÀ:!vjNR@ûHŠˆY«@À	‹û?Ã}˜F³B¸?Û[Ÿ"š‰¯@²¹šû@è*~XËs?ïÿy'3J°¿Õ:–9üÑ¿áôÌÆпëêry\ã¿êDå!ØAö¿ïÿ) 4ÓÇOTHERunkNVSS J175606-251909?†èãùJI?ŽvVHU?Ä7ä'?¾•<´…Ïá?êsëWê—Í?¿'ÅCat?'=iE¢€ä?äû³œâ?Ǚbk0"??¹û+S^L?鏼ãi?¹~;ɔÐÈ?¦"ÜgO¾??…‡€Ù?Òúª¸ûÔ?·×ŽH÷"?ålÝ
?·˜ À?fŸíÈ)u?QŠÿÞ¸ò?Î —%ÌÊ¢?«°âȇó?èa;2Ÿ/?«ÁÀ±S¡r4FGL J1757.7-2337?îJè$?×ó*š}£À8‹
É^çÀ:¡žJÙB@ å[ºà
@ä=F²kø?ÊQù\wÐ?Å*©÷µ®£@Yí{ì
?òe@çPܑ?Ú[©ôÓ?Û&º>ƒ¿è|X@2õ÷¿á×L¸?w¿í¿5դ⣿ÀS±OTHERsppSNR G006.1+00.5?‰øM)[ï?…žŒjÿ§5?̃qƒs?Ȭ	ºÖ]'?èhû½î•É?ÈÆsCöÜ?"P?Üք?#wQÉéy?Ë¢¼ý?Éþ2c÷²?èÆ	Ha?ÈÇp_ŽP÷?¶Z¢…Åô_?˜ú‡ÐÂ?ƹÁE¯}b?ª4Øk_?ç†;]Ûb?«±šDÈÄV?q)‡ÖBB?\ÂèP؆	?žÔ‡"µ?¯o–YÏm(?ë5÷ëqÎ?¯L­¡Mµ4FGL J1758.6-2404?ê<°E¾·¿£.y5}À89Vº øžÀ9þœCc@ äÄ£³xé@×î['ÍÍ?Àa×5†t¤?³sæÐ_~?þ>ɄBð@@ãJ膑ª¿éJ]ò#ž?î"Ó–ëip¿ê¦]¨R¿ÜÑÓñM5¿áçj¨† ¿í×ïunA&OTHERunk3FGL J1758.8-24021RXS J175835.5-240203?³ÒŠÞ ¯]?¬Ûbeø˜?° ¼õ{"?µ¯«nóDŒ?ëq—Œw´?¼A²Û§+?ÄxY¦ƒ]¢?Ä{n<7òÙ?©á.Æ}Ã?µüxUњƒ?éCÖ¶2À»?Æuìirì?É+ºE¸,?«å÷ã!¾Ñ?¹ÑT[WM?¥p3Œ ã(?æzæã'o?°³…ÀL?´ùO¸Í1?Ÿ»J°µ?¡{/C878?íuûAN?ìI#²Ù&?£v"4FGL J1759.1-2347c?î\ŸþÀ?OÃ%ãÀ8£hQ"1ƒÀ9Ò`8Nûç@ ½}mi
@"ã^߉h?Ô~/%1'Ê?Éèâ'q	@	Ãa@O?þþ¡ì#6¿îˆ¾ªö
?×ÒíbÄp]?ëéšbí5¿æ"¸žÂx`¿è³†_€>¿è-@ªêúµOTHERunk3FGL J1758.8-23461RXS J175851.9-2345110?‡ô«õB[B?"Rǎüd?¹óâã'ò?¿ ¿ÅƗH?ìa°ó¸µÔ?À"/"l×?¡›`†R?¥øÁ™Qù?¼ær!Çî?Ä)kûs?ëI{º®>?ċF‹²†Ç?±!EO'?¾‹!ö¨?ƛz$]?°æ"ä÷2?è6N>Ç?°gZQˆÊ?‰&…)9ÿ?}Q»S¹öF?šy§OÙ?šê6'(Ý?îÆ2€°âZ?œæ"´{]¾4FGL J1759.5-2312?ïD¡x=Ý?ˀæYæ¦=À8©¢ò(§À9ÐaŒâÑò@/°NÜ@ÒÇû¬´)?Ò`ÍX
?Ïϧ¹õ@	àÛ'£H?ýI"='Ûà?êo€Á[€¿èìßý+9j¿àõ\"•¬$¿ç÷ÆÀÄ*è¿æOæ'æ¿ïþ'!€-bOTHERunkNVSS J175948-230944?¶±MÐ{j¼?µÔ•ªwy?´ ÚÕ³¡?¶š¸7Ñ?ꕺë8<4?ÁpƐ¸,Í? a"䱁7?£!ƅ¸¿=?ªë!`Üè?¯71òú;w?íK4ϞÚ?²7z<²¥æ?»‡—r?Ø\hOÙ?Á9²Ò&93?¢pÅ'¯ê?èQ"Xˆ³?¦5õ®b1?pÒ±ùÚST?`<akê?•Ó¢«â©
?…l'7få?ï/½†­6?†š¶l‹Ù±4FGL J1759.7-2141?F¤Ð
f0?á)À8Ïa€M˜9À:ªh_dêe@Àîó[Í@¯…^y2?¼Ž½Gž¥?Ñ!šÄçÑ
@ÛHƒ&Ž@9Çóʲ?ïþ–Ž0Z¿çôÛߏG0¿Ùzßð&¿å2	g‡Î–¿êC@؍J¿íû,áàZHOTHERunk3FGL J1759.6-2141NVSS J175946-214231?± H,t&U?¤â¢v•lI?Êõϲn¶?¿mšÍ¸2	?籆"߇?À¯` §eø?¦06®¢'?¥±Ûõñ?±`€)Âø?¯yÆìÏó"?ìr\÷\՗?´ é±?Ưs={Ù?©-œõ›Æ?Ðè6ŠgÕy?°Ft ©?áàëmSM?±E¼÷O(?¦tˆqä?‹¸ÏŒx'[?¹ W‰ÂF?œã¿ƒüN?ëd¨æ@¦À?¡Ðâ#%J­4FGL J1800.7-2355?îõƒb—ò¿×É] í`kÀ8<Rô™špÀ9Øïÿ×¼@!º˜ó¬_š@(@Že‰?Ä6¨2¹°?²ðãB1h?üJë!L?úúŸ³ºC?îT)'°I	¿ã.ôàM/?ë^ÊÆbO€¿çSÿ[•R¿ÞI½ƒƒ­Ÿ¿é['£HoOTHERunk1FGL J1800.5-2359cNVSS J180041-235622?'ÅΈ>ÞS?±ðÞòEA?ˆš›—
Š-?"'Ðz%?ïR~W'Ú]?˜xH‹•>?£1|c?¨Ó¢®ñì?¢ÿHF Í?°*@i;²?íž,s³‡¼?µN¿XžÞ]?´ÅfZs?™KÖ»´›%?¶" .¢hÙ?¤ë÷J?ê"ß.꤁?§‡RŃ?'">ڟí‹?v¬yÒï?'äÍö1?"(Ïyr?ïŒ"ãø ?•"-/}êÞ4FGL J1801.3-2326e?ïjøŽ¿Ð:ÛGÀ6,l™†NcÀ8³Ïqºû@ »\æzH@B¥–ýÞ?¬¸oâTã ?ÀÁà [R@!,ÁÊ:KU@ºyŽq¿Ò1܆~3ã?ïsR4¿å•"õÎN¿ãÁè"Ïf¿é9Ò9¿âAî¢_ßOTHERSNR3FGL J1801.3-2326eW 28?'DÛTV:½?¿ãàHH?»°b†Ê¿?Â7åc¶Û?ë÷ÌãltÓ?Â~'d¨á?…™Kd=TŸ?N"¸§C/?ã¯waX?Ф"¥?ÙIEïR©?Ðb ÉÔå)?­4o@?˜ãýbY?ïÞ÷:á?ªl¯S…Q?é@÷Ï@m>?®½¸Îþ?0ê"TTÜÁ?(
+½y·Õ?ămåô(?±‰
#"ď?êüAà;øY?±Œøv½°E4FGL J1804.7-2144e¿à‹¹Ôøj_¿¸G7÷é=À7d/TbÀ9J®¯«SÖ@#*0oç@UhƓ?«R€o?î?'IR{Å?²?ïÝDêÜ0@Ë<quc.?ï÷Տ-Ú¿ÞY•‹–¢¿ç…=jĚ¿Ø9›aðµà¿áCœRæW¿Ðø3£¡ÂOTHERspp3FGL J1805.6-2136eHESS J1804-216?~üÃë™KÝ?žƒ.ˆÅ^‰?Bq¬,Q6?_\ªG?ï½j
¹? 5#T—¥?™[]S>ý?¨V5ėŸ?¥Û¬+p¬m?°U!ÐY
?í×lâ^[B?´~£`¶•?¶0¦AŠt?5"‡œXh?¥¹ÙuÔÈ?'SÀ@ý÷'?ëÞM qpB? òŠÄøe?kÿÝÈ&?a¢¬Óv\ù?‹Ì¼Û{ў?'¨*äÏa?ïtÍor2ó?ƒlr	1|ƒ4FGL J1805.6-2136e¿åλê§SA¿Êó› ­JÀ7cÿ¥g-6À9A¹d:<<@ Ðyšu·'@žš|îh(?·6=>Nð(?¼¾-]íWB@*{[Àðö@åŠÞÁ?ïûþQ)=¿ï÷" fQï?ï¹ý‡»¢¿äˆk%^¿æ.oŸJ2©¿â󵤒 OTHERSNR3FGL J1805.6-2136eW 30?•t†9ä(±?¬±ä蒸Û?ŽÜA`´‰¦?¢¹O#ԝ?îØêÈ®"?²´œÖöÜ?Þ@\>Øb?¤óŽ÷I¬?¯?Z!+¸?¸i†`±ì:?í'{ö€?ºdŒžC"€?¶s'ºz¦7?{H¾œq¢?µ"íÊÐö¶?œ0ð~Âó?ê/ïVŒb?£²H	ÄMy?k·‰9Ù®?gÆUM"~˜?"Fy~?˜N['‰?ïKŽBý.ç?™Õ¸ÕR4FGL J1805.8-0803¿±*7*"@UÔ¥ß":À9ůJÛÆeÀ;Šꘐ@&¦7aÁ@Åêû‹üù?È}ë=PBŽ?¨}¡%ãr?ätÌ?ß ?ý­:`N?ïû¶Å#‹ ¿éh°B¨q#¿ígB'¿ÒùsÍÅ¿á	²Û‰ÿ¿ïÿ‰kVOTHERunk1RXS J180603.1-080612?Ô}]L¤?Çìå'MˆL?õ7eă?‡~ÄiO.ç?åym|`?È("'ŽM?Ô«äŠYõM?Ä;؜Á
f?¡øÉÆ«Å?¬Ñngü›?䊁rڝ?ÃEcs³|8?Ù§KCw?°²–ö®u?²ŠS£žq?–4˜ËõÔ?àé)Åv?¯¹Á?Т	µ1?´Föîíæå?šª",¯
å?‹~J#
?æÙ¦Œ‹?µ5'u¡Ž4FGL J1806.9-2455c?íŸë¤mÀ¸Ðº%*À:o1çÙÀ;|`¾†¸ì@ÜHjÒÝ@"Á=L'©?ÔjßÇÑ:?êê!ƒ"@?úÁҝÇ@³+XžQº?ؔø T‡¿à39žeË¿É) 7mŠ¿éGF{"¿ïá=¼#1¿ïþ¼3!•|OTHERunk3FGL J1806.7-24511RXS J180700.7-245619(?ÂP¸y¾V"?ºí%W­?´w9–¼%?³.tã@ÁB?èÜê¾]'ó?ÁMk€çlÐ?º9:K·W?³¿A1EQ-?º×é 1ºõ?»"œƒm?é]ے'ض?¿ßAáÑÏ?Ó3¸
M4?±lhÊoi?Ê2èiO?­°Î
ۀ~?ß³A~~9L?³$)ã"ô?ÃÑCü͕?¢¢®Þ§Ø?Ðyk?±Â@Õ?ã~çKI?³1ƒ-,í?4FGL J1807.8-4340¿ê˜EƒdEqÀ&G2œ4~À:4I½¹3"À<àd)u@§ÏBrì@ùœÝñ¸?Ãi¦!gXÕ?Ô'r 0Œ@
NHboa?ú:š³JÕ?ïù?†þŒb¿á8ýw"¿ÛxŒÙ—¶k¿ä½þ}ÉÚT¿î–q[Œî?"E©'oÜ\OTHERglc3FGL J1807.5-4343NGC 6541?³í'»gN•?°" irMn?°ebn ¥(?«âb4§¯?ëu®º¿ˆ?¹_I	?âP¿á¢d?Ì¥nøJÌ8?Àњ¹G…&?À°'weŠ?Óp'#˜ø¦?É[ÿìµo?Ù©VHÜA€?±Þ	)¬C?Ðkwö­™v?¬ßN&™3c?Õë1Àv%
?­¡;
z%+?Ú¢	ÙÚ4?¯>øæà?ÂV3'"?§o±¥šg?Ü2Ñ5¤]
?µñ¯&i­4FGL J1808.8-1949c¿ÝPxυË?]ÐСõ\À8ˆF"
qÀ9¶¡Ú°»@ –îE1b@àM/^?ö£©Ø«þ ?Ôôqâ'Ò@Ãñ[øN[?ø±÷¤;Þþ?ç:¶#£s?îêÖ£d!¿èÛLAw»¿êKåM¸¿çqµºa>¿àÂç 5)­OTHERglc3FGL J1808.5-19522MS-GC018?¯.-ú6»?µ¢–ìšÀú?×åxéðóá?Óʌa;Î?â`ºwâ¥?Ô'ª½Nì?˜~ð+ڙM?¦CÚu3i»?Îtn+˜õ?Ï)øî‰tõ?çžìóºíî?ÎÜkQ+ö1?¶ÖÁGV©è?˜Swm³?Ëò;—±{?²
£ªgõ?æ(¦ˆ/>e?²ükt9åÞ?w
Záè?€<Õf­Õ?µØÔ°Tüû?ÄZ\‡"lØ?íÁU?œ?ÄiçyZÒç4FGL J1810.3-1925e?ªÿ¸wRM¿¾(w~¢ÙpÀ7±C΋é®À9"y
2ª@‰Ä7@Š|Æ$<?À<"·Ÿ¿?ÒEkD¸Ã@¼«œÑ\@Öªß<;?ïë>bk]¿®w9>ÝW׿ÜèƒažÖo¿èPÄsa÷l¿ã#Îq»¿ïôU§ÒAOTHERspp3FGL J1810.1-1910HESS J1809-193"?kê–7)¬?g¥[h²ó?'hêÎmŽ?"œî'ßþ?ï›ÏÆÀ ?ˆ+l•õŒ?'³l‹(nÃ?"/·	Ä]?À&ÔDþü?µõ
cvoI?ëh¯Šfý"?¶Ôê"Ô?«(›¨Æá9?'qŒEge?ǪR•ð`]?ª9oªæ?èbáŸ÷yÔ?«JzÛ
Õ
?iÅïLÜ?`ðôÏÅ?¨öFu:¦?œT.CÖ?îVքÀÆ?á$Îg-œ4FGL J1811.5-1844?渥\Š3d¿¤lי¯iÀ8EŒîkóÀ9ã?¹SsE@+×IR"@ŽŽ¾tDu?Æ­'@
Üþ?Ý$)à¤&@ž¡aä÷f?ý	ø`Nt?ïû1~þá¿Ùv}_Ò"¢¿æ"ù2e-¿ê¶CŒ¿ïÿýF\I?ïÿ¨âaßnOTHERsppSNR G012.0-00.1?Å'àHë~!?Ë!f«Aª?¹ú<×?d"?»¼rG?QX?çvÀRÝ3å?Í½—±?¤bo)9¾û?©×õ߀?Ñäg"ùÊÜ?Çs£ÔÄu?åÇ¥{ï~£?Ç2&Z
?½ӌòå?£Åñß+òî?É!씇i?©(˯ãa?æêi?ùi?®þˆWö?bÊ#z ¬'?ResÅ'Ü?ÉRہv"?²÷ÂT?é¥á%¥¯?²$ÒÛΜ4FGL J1813.1-1737e?ížñ•·•a?Åæ­ýÀ6…Fü=ÔÀ9OVcÉÔ@f€®¼š@T¾ÆyÌu?©$S…í?Ã@y—Ɔ@µKHÓ®h?öf¼ýÌÉó?ïÿ@OÁß¿Ò2l"¿¿âµƒž¿åéҁ—š;¿çEsÝGnT¿ß:md1'ÚOTHERspp3FGL J1814.1-1734cHESS J1813-178?"WÒnp¯?ö÷¶Ö(?rëöf@xT?w3'¬,*ë?ïˆÈÊíÅM?ˆ)׆»ÆÍ?YFÕö?‹ûÞÄD¼?ãÿ‡øWø?Èh¡nz7?×xµDÑ`?ÈcøÔ4N?®è_JäÇ?š·X¸\®~?¿ O"*)L?¦0iÊg£À?ê*÷‡†‰?¨âýh1YÕ?Sc=õÑ&'?FíÇÿBƒ?ɨ­­ù?·…ªz?é±d5™¯î?·«ÆŸÄ©94FGL J1813.7-1536¿ã"®~5Ï?ðŽw&¨
À9rp·"@À:¥Mçê_…@ ^)dÓ@Í`ÛâêF?Åꐗ'X]?.77¸º?Ï8ÿ%­B@Òͺ³p?ì/8"9³¿Ý#÷p"¿éÿJ-J»æ¿âåPQQ+¿çB:73rô¿Þb'|,OTHERunk1RXS J181335.6-153600?ž5,ø=?—žþ`>?‡¢Zü·?Š·<Ÿšÿ?Ì]ÌK?Ÿ{Å¡´?Æ"#T¶&?Ä(­:ÍqÉ?ÜÎ)8?›ÕCìk¡&?éøã†Å•?Ĩ~'ß?Ç>²]ý½?¤œXM‡?®z;¾"
+?É?)êÈ?èH¯¬—~?¤½ñ"
Ïi?¼¤Á¶Ï?£TÊE}ó?…y¹¦Þ?qÈC[X?ì˜ùäâŒ?£¬Jømp4FGL J1814.1-1710?äDñàhÇ%?Ç	j!†ã_À8ò(zrÀ9þªhö‹@ ~JL)@¹åi|?Ð23Xòà]?·åΑs?ñftù§ k@½®€0'î?Û$cAmހ?ìÔ_¾+Ÿ@¿æE^XûÅ¿ê)óÿk°}¿Û]"3¿ëBÇû¬´)OTHERsppSNR G013.5+00.2?Œ^¸c"?†{ç%?:?‡Ø€ò;y?'t'q§â¼?ï/#cäÇ?™ŠJ׿€[?²¿\vŒ`?³›Y¥'[˜?™õ¼e€‰?¦î¿h˜·?ìØdŽo?¶2jWéñ ?¿Ê:'Gj? €¸ŒÅª×?¸ÍTýÖX£?¥nö%?éÜKþ?ª´(ÎÌ?¨ƒ'R™½?—ÚÖ{—ƒ?{ã9f>/?r¢HìÙ?î@Îc—³?™+Ïm.:¨4FGL J1816.2-1654c?ÊfW'¦¿ÁS|©É½yÀ8FñTk'À9Ñ×rB<»@Ô_¾+Ÿ@Ä[^Ëgr?ÏJ*,¤N?ê[éhÐú@-?ü¿ÒxˆQô?îê?¤Z¾¿Õ4Îÿ,¿åÀ ·/¬–¿îo/˜sÿ¬¿à± ‹ü"%¿ïþLké]&OTHERunk2FGL J1817.6-1651cPMN J1816-1649,?•×ë©ê•?š=u°'ù?«ž$ñŸ´?·ŠLÛg?흎þ³–°?¹Õkôt°¹?›&G[½ë?¡•™B—ÎÆ?̕«¾wÓ	?ÆFž=p"'?èbՄå?ÅcmS`ç­?°³'ÅÎ̺?š
Y=e"C?ÂEȋ™?©~Á±?>z?éX"_à¢?®³iŽ	û?Põ®ðlrÒ?AZô…1±5?Ðp?–ùC§?¾­¶l?ç¿e]'ó?¾¯"öB4FGL J1818.5-1656¿ž(Y·íœÅ¿ä¨ªxäî,À8×£Z»ÐÀ:^xèI*@ûÙc¯@÷‹7GN?ÆvÚèCuÌ?ٚcƒˆ
P@2 f<u?÷úÿåþÍ¿ïß4Bý«'?ïû>?*ã.¿à¸Gڊ%¿åz·\Ç+¿ìӋ,ïLT¿ïû¨LºÃ¶OTHERglcGLIMPSE C02?|—˜1
rŠ?uŠÌx'›€?²êÃËɝ?µ¥ƒ1'~u?íixn¤kç?¶MË'Æð?˜µM±8S?šµçŽ,À.?Ò*'Ç[«?ňAџ?æ%A®Édè?ÅReü!<?±hŸ)~ÍI?×úGöæ?˽¿U?ªÆjg8òä?æ㧓àe?«ª
ê?f?ˆ§Ø›«?tÝ珐¨™?ÇFòö)z®?³"¨B?éÌÖ>æ?³ê`R!J£4FGL J1818.6-1533¿îb;qáÖ¿RnóÞ)YÀ7^²²$«À9^[ÿÛ@"ú%u…h@;¾òïv?µ7ƒNÿl‡?ÒÿßÝ5¦@1í¿‹›ª@‰a´¥ä?ïÿõ4Ê㿽ë *F>¿çìÞ²þE¿éçÑ—Êâ¿ëŽ5Lèæß¿ïÿò~#¿OTHERspp3FGL J1818.7-1528SNR G015.4+00.1?ž·œÙ?¼az'ƒœq?´Ãšß!&I?¿[ˆÿÞ?ìqÔ6û?Änfu‹È=?…È=NÉ?Ž§õjÊ?۔Ÿ¤ª?ÆûŸvš>]?ááÙ8o?Æ 'ä}T?®§''(*?š•ôÅÊn?Û¤œ&±Â?¸iÅÎn?àC'™Ä"œ?¸NRñaØp?D²`‰fâ?8
‹e,+?ÆÿŠv¹ˆo?³dV¨fÐ?ê:ðÛ¹{Š?³rέ.¦4FGL J1820.3-1009?²ù&oÞè·@zÿèƒÀ8òdtJÀ:®nƇ8n@x±Ü¤Û@^YåN£Ò?Ç=|!äI?ÒTÕd éo@KBôqW?ó	Gðjâ?ïÖ8ñ¹`¿É68¡1=¿äÛ
bY'l¿åépq'#[¿ê#u –
¿ïÿð懈öOTHERunkFK Ser?À6±mŒŽ¢?²ãÐ
"tX?ÓÚO¯a˜Î?Æóé¦)š"?â+Ììñ?Ç`_HÌ#]?¡·4$yï?¦|ôڔÚc?Öy¾åi'?Ífƒ¦j¸1?ã¨ÞE»)?ÌîÊí÷¹?Á\‡A»¤? k,k>Úa?ÉOé"2y¢?©¯°ivϹ?åTãÖ"ò¯?¬"Bõë?ƒÌL}?li4oN?Ò•f41'?­Åå{X?櫚œµB?­–ècÎïb4FGL J1820.4-1609c¿é´HãYè:¿å^®óÀ7vÀ#jÀ9ªdÜ"«&@lúnp ý@RnÚ©.b?°Wá&öå?gêfß´»F?³£</±š@Ý<¥wÉ:¿Ý	üƒ×+¿çµv¿åªÒa6PÊ¿è{:3µ¿ë¿Ôj³w"òOTHERbinKleinmann star$?¡‹].€ÙÚ?ªsœs&8?xü,X¿y;?…¾U‰¤^î?îµQÔfsp?¬oV–Ó»÷?ÏÐê²½v¢?Ê<­k>A×?£Vߍyõ?´Ò«ÏL~?æÖWZy?Ëâðéi;?Ɇ!ÙÎ?ªuš¨³¯?½Ñ6Ëì!?£©@:Ā?åþ·¤ÇŒ?°2å\›Œ?´­­°Ý?¨ð(ðô?•ÔqßTR)?‡eRh%y?컦»Ë?ªàµTâ;-4FGL J1821.1-1422¿à×3}'ju?™ÎWçG¢VÀ7"H¤´ÏÀ9Y{ÕctD@§i&à@M¢ÝåùÄ?¹Â|ò–‹?Æ®nþ:ƒ	@
ë€ìúi¾?óÒÑ=õ®î?»›Ð>ò.¿ä(@zi¿æ'ñ.«äö¿êAyHªi¿ëát#¾K¿á»]¤ YOTHERspp1FGL J1821.1-1425cSNR G016.7+00.1?xŽ¶—Cû?{G‰m<†?œM­ÖjT?±é㠖¼?îìu*JƄ?²PŸ"[åî?'=6åXŒó?"[+Ñª'?ÂMþxÍ{R?»IÑB/?êږª¡ÜÄ?»/"#ÿÁ?½TÙêÕuP? ïÔÐ}?É­îéC­:?²&Ÿ<	Ç7?åééTf?²Ôò	¤¯‹?Vo¦T¥á?LBF–Î<²?¬Ì#Â{5¤?é{ÂfVb?î(2"R?žÆèŠR4FGL J1821.4-1516¿îï
øÍAù¿Ý5%:ÍÀ8Iûçl‹DÀ9¢*9mÇ@Épgq(a@ŸGù"Õ4?ʹ~%õ²õ?áõ£àðEM@Bþ'Q@ïƒm2?ï½'"ƒ¸‡?˜hÀçCú¿è¢Ë§2ßP¿ëW*ß&Á‹¿î˜ìËoÕ¿ïÿA"VOTHERsppSNR G016.0-00.5?h^µÉÏ?i'kð¯ªæ?hy'<ßU?q66t8ó?ïÏmv
V?y
Ê`_p÷?¡ìBæ¥j?¤Å	õy?À÷/^§:¿?½`ga›ÀÚ?ê£oùôFù?½}
Ýßñ?¸Ç""ØE?,¥AÇ,?'n*ëY9?¥om©`ø?ç‰ü`׳?©ËÐú•=?eTO‡M?Y³^Ÿ!ƒ[?¹ó•]ølW?§PÒ±®?ì¬9-æï?§»¢+Ø9È4FGL J1823.6-2345¿çÜ[ªÏÀ'ÛŸ'xÀ:&Mâ"sÀ;›mB"º?@Ã=¾Q‰à@;Û¾Ø?Îø¾'²!{?Ѓբ‰WW?ü'à@bMÖøtÆ?îøçþ¡f¿ç¼]éÀ#¿áä=Çᬿãù2±-4¿á_Cr¿ïø°ëŶXOTHERsppSNR G008.7-05.0?×=Ô{íxõ?Ã断«€Ó?‡ª
'õwú?€Ý|Ý¿¨?äm™im¦?Ä%¥#á?Ùä.,o?Ä9žp?{ÝèO"²‡?‰òú<©¸Ç?ãAÒ.ÉÀc?Ãþï2îÑ?âX‹ç®…Y?µ6Ïì¦ã?­Ú>Çn§?"è(KP?ד WÀG{?²ÎLO1
?ãh|ur×í?«/zž"x«?‰×ÅJa+?ts$X°Û?Ø`HêÇFÏ?ªä¯Ÿ˜274FGL J1824.1-1304?鶚wÔ¼Ÿ¿q™JÞ-näÀ8ÝäLESÀ9'ý÷Cõ@ÁªKÃwä@|5À¬-?Ëó²ª6ÊÂ?èh(=5ët@"£Ÿ¬Ù@i'|'v?ïøʁ˜ñÔ¿Þ1›cHNοç(¬âKº¿ïÿ¨âaßn?èÉâÂW}ë?åÙÑ,­ÝôOTHERsppSNR G018.1-00.1?­m8%´?¹ˆõo%•?‡O_/Û	K?˜L¶çÈ»?íËïîÒ??º»•õqúô?½V[ýÅ¥`?ÄSUtÊÙ?¿
4~«ö?Åí¼®é?èsðqë?Ë¿ãµ»€?¹ìì'jã–?¢> șx?Åœ!Q5/?©§Ž¹ÇÇ?çz»g^VA?¯ ˨?"—܆¶z?‹f";{êw?°%/à­ä¨?·¼9Ÿ‹Æ?í¨ýüx('?¸5å,ìåÊ4FGL J1824.5-1351e?Ò0§"ÑU?¿Ý6syÀ6³"÷si"À9N?(3ü@#›Ÿ"X·Ò?û¬	sFHº?¤å¿b%??‹R·ƒ#?öŠÙv0@äÖ¼9ג?֋Ⱦâ(?â6*~®±¯¿Ú³8ÜÀ_׿ØcµÜñ22¿Ùsßà›¿ÌÚeçr~OTHERPWN3FGL J1824.5-1351eHESS J1825-137?~>§Žq§?¡Ã6Z½»Ã?@Î)ÍIF?fDdR
Çß?ï¿O&pvØ?£#ž¹»¼?¥Íöå7Ä?­:"+mpk?§HÃ-Ý¢®?´›¼ðÿk?í.¢M³ÒX?¹Ê‰»£>?¹íèŠÅ?£*q‹pIŸ?¡|'öCa?Š`ù›˜º?몁æßC&?¤v
XyE?'ƒvjn6[?ƒPké(y?¢"U…å ô?—¯B{Uh?îKžôN<>?š`\ÃmT4FGL J1826.2-1450¿ØË«@"¢¿ô¦D¢Ç?ÅÀ6 a3÷À9i£bp7¡@ãR™€@J© öÍ?–\Û£)eT?¿gûfé2@ ¬B 6m@›6PtÀ¿ÖdΡ8Is¿ä ¹ÿȏ¿æ{4ßZÃñ¿è›Ù°
g¿ìwQ­Dq¿ØÇ¿Sg†OTHERHMB3FGL J1826.2-1450LS 5039?]ƯÿS±÷?V—"¸uò?oóoeãI?v#*í'¯?ïÒ´ðD?yу{?–£×ø|^F?¤›ä%6?æí˜Ð®•ï?˹š7‰ù©?кß=?Êaäü³´J?È@œYpq?ªÏ­§¾?чßÃ..?°Ji…šÝq?ák"ù¾Í?²-b‡ì?h¯ÒaŒÂ0?ZEŽÂ^A?҅ÒJ"·Ž?Á—©§G?æ¤gTv?Á£CxEVÀ4FGL J1828.0-1133?ÚOqèOµ¿ÂfS†ÑšÀ8Nµ‡5éÇÀ9îÐ_(""@&Þ÷q@ö¥†6æF?Ä/fÉû?âtöL"'@'5Ÿôým@eãmx(†?â ÀaŠ	?ԋ"|I&º¿Üi'ûr}¿êfs.ËÅ¿îrç;
¿ŸzSƒ4ÓFOTHERspp3FGL J1828.4-1121SNR G020.0-00.2?WsV¿ÁÞ?Pv¨.žÍ?Õz%?ÀRêÏ2êÛ?ëçÓ×
[?ÀXiaÔ«?–\=µžˆ?–R*W'*?Óå^°X '?Ҙ©¨?åZnº&»w?Å3²¿q%£?¦V@Dz?‰»â­Ê?ÖôiDô<+?´q»^Ù?ã i«¡Ý£?´ŠèäŸ*?pTNÊ
Åó?_ëlr?ÈawÔÞ÷?µ.7Í®?éÆùm4c÷?µJEånt†4FGL J1829.4-1256?ïë¨Ó{ñ¿ñeªIFÀ9cQ³PúÄÀ;ƒ:=°@¼]¸ÂÔ¦@"¯ûî|?ÍÛ`#`"?ïÛ}i¸*~@õo›Ìz@³ɝÃJ?ïƒ{_œÈ£?ïÚËB‰Œ?ˆ¢õ¸ÔG¿è¹"8à¿ïþ>>ª	Ô?ï¨wÆOOTHERspp3FGL J1829.7-1304SNR G018.9-01.1?¤¿zoDÑ?°yÜd'?ܵ¸ø;x?ÊúñcŸœf?àY,J•3?Êä:@'»(?ö=.©Q??›€ëí="?萲Ѯ»Ç?ȶþ¾ýZg?˞moæ½?È,·Uó"?·8™WǬ?™ERy]J½?ܙ¯¤?µ™…©?ݘZ©_U?³§S®ç'?vÂl{ë–?p;-Šùbp?í»/ß>©^?§íþ'uæ?°ÅTßBö^?¦‡®Fm#4FGL J1829.5+4845¿Ñ³.Áž@7Š\å´$À8¾©@'À;ûl'à±@B˜*Þ@ÙuòËd?¡òœ*'?¯'öiÿ"5@êeÀN9@ë財*¿ÄI'C¼˜¿âßwßµ‡·¿ç›˜w[¿ã".ülοë€JœÜD¿ÞU3ÃÑÑnOTHERcss3FGL J1829.6+48443C 380?ï .ïM>?b[zí?f¼à'®g?`=f'¼ç?'EïÁ/Ð?{FÀí¤U?ïwÐr'Ÿ¤?"Û°ßà¿?cF$|¡P?wÅ=´û¼?:Z<"îì?'²8€Ë?ïÂYýÐ?‰'.~}tç?€zWNqi?}€ÏEZŽØ?•*‰4õ
H?'›òÖÐr?ï©
É9,ž?pÌ]Ly©?sn~ˆ\?e§ìG@]©?x
œÛU›«?cª‡¹A4FGL J1830.2-1005¿ìصú.&?«W2"Ç{À7×)ž^û8À9""išÎ@¢ÌÉè>@
Å㤀?ÄA¼bò= ?Ûæ€<¦N‰@ÓÖ¿•?ôÈ[á¨&$?ï±½¢bk¿ßZ¿žæàt¿è˜8p‰Õ׿옝?ìT'¿ç?Ô@ßn:¿ïÿ·ÀÌ
ŠOTHERspp1FGL J1829.6-1006cSNR G021.5-00.1?€b"y±å¯?£ƒÀìÏ®?ŠR›ZQ?•øš|‹G	?ïU/7âË?¦™­ÛT©ƒ?ŽZÑÀý
?'';éwݤ?É>	•D?Âq0 =?é67uVº?³@ƒ"?¶y5¡{?Ÿ¸"u#Úì?œѵW?¤²ÒÁ
þ?è‰×êïÖ?ªç
Ï¡Â?D"Rîtnã?5úf²ÌÇ??Æoɔ¦à}?³c¹ø—Î?ê^èƪÄ?³mþ÷µ—F4FGL J1831.8-1503?¥Ô"HJ<QÀÈõÝgNÄÀ:™ °åºÀ<RG—nF/@ÐõLrÊM@Ê}Å'¼Ý?Õ8¥ƒ1Î.?ïý'ÒÕûJ@ÃC·õf?ü€Ó6ô2í¿µL+@V?ê?ýkûý?ä`s^™¿åª%mwҟ¿ï$X*Ž¿½pc×%ÁOTHERsppSNR G017.4-02.3	?¯1«òýüÂ?¦=³¿Ü?Çb;Ë?¿·e/ðã?è4c2YA?ÁÀY5'ú?³Ì…Ü(#?»æt¿:/ã?ÒÿK!à(?Îò01¸B?ävo·ÓŠè?Îe¼jôô?Ü
±H2?±Œ®²NB?ÍìKãI^ü?®6ÍC©†!?ÔüÄ]f?¬85"ì?¸"Ü×5~Ö?¨ÝñÊф?èsô¿Ú??º•¬µµ?¾˜Aז?²¥Í›a4FGL J1832.3-1433?à™Ñ'¯D§À¼,†pÇéÀ9ÌEŠMÌ<À;=5¾(@]l²ŒÛ?ÿSýÈîû?ЉCá`x?ÙmR=åhÐ@ø£ë,3@À<-'Å¿ïxvétù?ì®ç¸5f?ÒP×Þά÷¿çŽáDS(¿á4&¾Ýà¿ï÷åê«%OTHERsppSNR G017.8-02.6?Åg¸€´B?·r1s"}ù?"»¥Ñ®]·?•>4ð?ê>ãR`?¹[+1,F[?مÒ"1?Çt­œàîÏ?}J•s")?…ÆºXš.?ãäÊÎÀ?ÇQ£ç¦dü?Я}I¶:?ª_ûØ<g&?Á[¸'"«?¡¬ØXbR?ãc!S6¿¸?­®I‹n"?ÜcP?ºå¾á
c?–þàÀÈ7+?ŒY)hþVÓ?á?WntB?¼26½²MV4FGL J1832.9-0913¿éì'£lg¿ÁÁ›o¨ÚÀ8Ó^R›®GÀ:†••þÚf@h'Ô±Ã@û]‰H¾?Ìwt«£‡Y?å·Y}ʱ@Q['—@¶HW²™p¿ã€üŸxUÒ¿×xû~æåÓ¿Ôîÿ&¼,l¿çXUÌ»/¿î–÷'ê)Õ¿ïë;³´MOTHERsppSNR G022.7-00.2?…X¢à9-Ó?}u™Îä|?Çîo"Q'?¿!W$a-H?鯭å?¿€¸Ÿ8Å­?•Ü9ع?•Ö—ü¬n'?Ç¡_á	?Àçl»'Éý?éhÆvpý©?ÀÐ|'³T?´ŒS«ºÔ?š×à&¸i?×¥°AjyK?´ö™Ew?ᛣôÕL?³<'5_V<?…ñ¯-HÇ?q½lw•?Å"«§'<?ªðCNGyÉ?êcÔYfŽ?«N χx;4FGL J1834.1-0706e?ìâ
?âºíÜçÍÀ7‡†Nc:bÀ9÷‡©­
@ ºÓ»ÔW@B¤¸±?ª6CM1·?´¯Ï;#@½M%LÀ£?þ8r_˜ìË¿ï}1NV¥(?ïO¼5¥Ô:¿Ø_~Øտܳ@S'D¿ä…|áÒîO¿ä˜…2ˆKOTHERSNR3FGL J1833.9-0711SNR G024.7+00.6?³šøueà?«äÈ7_	?Ã¿§°â°?–`'´ZÙD?í'ô¼ç?°å9F£nÅ?²$؋X²(?¸_8 >h?ÇpQ·®?ȓ¬œÖ4#?çßP€ÎIÏ?Ɍñ̽‹Ê?·ÕŸ"?ŸaÕP:Ç?³¼\ö"jê?žç‰dÊ?êÀ~,p?¦K™tÇ<?¦ÎÌ,Jêh?–@éÞن.?·žÝ#¦ô?¦µ0ñ~¬O?ëŸPA–Ü|?®–|BžÏ4FGL J1834.5-0846e¿ÖÞ˜•/¿ÑêÛá<ÆZÀ6øêúÀ9´ëvÛÿp@!q3­ª@øã["‹?©ãZ> 2a?¡7ßÀD~4?ö˜ÏTf‰¢?ðX#…@FA?ê!j³Ó¿×AIÌR¿Þ|cÓº¿ßü
1¿åèå1G ©¿Ö¿²ÝãJ"OTHERspp3FGL J1834.5-0841W 41?'ôø!nÜd?«¦Rö6‡?pß÷bÞò?y	ùUÙ?ïH2Ã_?¬v°Ä[P?‡úFL¹V?"Â+
¦"!?ǦÏÏ<j?ÇZP%â?é¶bóײ"?ÆéÙÚéS?±(ac-Ô?˜±ÛêÂÙ?ª€YÕæ'?"Ý-Ül 7?ì2êÝüç? Í#HÅ?p¬Ö¥zl…?c°áëŸ2?¼DU°YX;?ªÄ~7»|Ã?ìVœ©à?ªøwÅMdD4FGL J1835.7-3258?"QìÙH
zÀ&¼q'êRðÀ:"¾@BÀ<#=,±8ó@³7ƒ$O@Ê#9Àëî?À‹ön?×ÍýNtØ@R° ě¦@J~}"N?ïÿ?`h¤¿Ã—Ëù")h¿ãmß âM½¿äQQ¿î;Äf̽³¿ïûç6Û^`OTHERglc3FGL J1835.7-3258NGC 6652?ºßhµC$?°õE9æÒ?è	îq‡Sç?À"ʏ^À?Âh'.ˆÕ?ºVÁ¸^ˆ?Çu 鲡?À'£]—h6?âÑr•µ.˜?Ǽ"ðþ'?ÍE¿yDþ?ÂäçHµ+l?À©©o	´è?¦"
¬n$?æ>½Ò‰?°uÎ`ß:?Ç9•ÿõ?¥y…w¼?љÿӈšý?£H_}`^Y?ÜÄ UE|K?¬+žÖdÌ?Ñ¡ß×1è·?¦JRqWæ4FGL J1836.1+1143¿äSkî¡Äò@!\^Ô¡­dÀ:uOøÃÌÀ;ôWVP@Iބ…5_@Úµ€í ?Í°£vg:?Ð#Ëâ5!@­Ácâþ?út"« «¿ë¥C¡?€I?ïôἩi¿ÝCm¨z-¿çrº'Gm}¿Ý‰šÈïÿð ¼x—OTHERunk87GB 183342.2+114143?Ù¦1FöÐ?Á›kÔlv%?°<ƒÒ2Ë?§•º	Y™Ã?áeVâ>??ÂKóêM·J?á÷øz"'c?Ë­gÚÖ>?¹Æþ²†7T?¸2Bh[?՞O_md?ÊháŸ}?ãYÄ^-óR?­&Æ¿5"?·›ÕÛRٜ?›Ddi Rú?ÓeÌÏbö?¨°‡{Gý?à¸ͯ]ú?«€Î![`w?´õÌÊngm? µÁ¦´u?ÙR[2ª1?«J†œý4FGL J1836.5-0651e?ïÿúr]¦µ?ÄCO¢ÝÀ6A‹sf)*À9"Â(.s@!&¤†‡™@;ÌDÑ	?›2Gk'í?Œ8e!Aï?ñ8^€¾×A@9nY$¿áµþŸWɖ¿–¦…Üàc¿àÔ*ÄϨI¿áÖG4q÷"¿âÃai&Š¿ØuØstOTHERpwn3FGL J1836.5-0655eHESS J1837-069?˜¼\&8x«?³DüvƗ?I•PÚ'ê?VjŸÙIè?ï3·Ê—»°?³d¹£{§?¿J¬m0µ?ÃJw¿šØp?»_þ
±•Æ?ÄßPSB/?誼I'0?Ê]¢"œ(š?·HüÎ? ¸Ø;b¡?ª/1ºRc?"ÝùòÉ?ësíJ™wn?£Í»ûÕþŽ?­=¸äÜ?¥5q:Çj?µÊí÷6™x?«	R6®Cù?ëvže˜ž"?±¤'14FGL J1836.8-0727?ìF6ߞO¿Æ¡)ÛƏÇÀ83È-*ÛvÀ9õ}å-@¥ˆáe‹@8ƒŸ\Q:?ĆÒíx=ÿ?ÞYG™ò"í@I[»èxû?õŒ>Ù.°¿Þ†=0âöÛ?ájÅÁ?Ðпáµ'ÿùJ¿ê½®ˆ*Ü¿ëleöÕ¿ïÿð°×£ÀOTHERunk0FGL J1836.1-0727NVSS J183652-072453?"´äci?¦€©cnä?Ϝ¾öcÆ­?Ç
¿'Øú?çÈanՀ±?Çaå
,<a?'T
î"?ŒÃ£W¼\?♏eO´ì?ÈUØnÑ0?Ú:@½	"?Çö?ÔYøk?¦FÐn×Ó¯?¹ 9–ÉÜ?×ÏvÙYù†?¶þ)C†÷?â³×Œe†?¶ÝñMA?SA¶âêTO?@ïô6gnn?×â=IR'È?µÝÕÄ"~?ä@åAr?µèLÔpû•4FGL J1837.6-2904?âKý¼PJ=À$"¹,HÀ: š=-‡ùÀ;ÞËêN½Ó@¢Câ-@Qš&‡S?ÌÇ`|B?ÝÙoØ2@4f'ëØ+@	…nVŸÉß?âó\²¿Þ¼l—ØÏ:¿äJ½"s嫿薣L;¿ã%žÀJ‹¿ïÿ-<y-OTHERNOVV5668 Sgr?ë¯	?ºݟzÙì?¼?† ¨
ù?µFTäåŸ?§&}X>?£ŠÇÿ
Þ?ßh5"Ï•?Ϥ[ua)?Ä]$‡ª
Â?Æ8/q'ûQ?Öi8'[d?Ìcä°"0?åE¸B?°ÑÎt?Á8ú=?§Ç±~";M?ɱØ퐥?¨Xcg+?ß-Ê(®_m?²züB!7?Éϙ€½f?±+dcØB?ÔGÎ
'Aß?¶ðiÀ3£4FGL J1838.3-2148?êÂú¥fñÀ‹;26À:h Ä0FÀ;딾h…û@Tñ¡˜kœ?ûžƒ
f?×µ˜ñ/?îªâ+Ù¢ž@&ó|cþ­?óZ…tɀ'¿éK—¾":?ïÝIúÑÿå#flE£x¿Ù££Þ–ú¿åñ0ߛÜj¿ïâÁáaYaOTHERunk1RXS J183818.2-214857?Ռ3b+þ?ÅFv2Îßç?¡»EùQÄ?ŸK	§íM?ä1õ¸Tå?ÆJzª¯X?¿K¡òXPº?À¶ P(²?Òæ!ËQƒ?Î ­Ò`¢?â£zÜ4e?Íԏ"£ø?â'1èz?°²-•÷/ ?½$²\UÄ?¡§FHq
?ÔhxC1ö?¬¾ Á±.?Å>±&"v?°NbÅw?×@=8䘹?ĵŸ¾ï?Þ j3º?Ám›¢¸`4FGL J1838.9-0704e?ïÜDU‰8<¿Ý¿í@_Á‡À7c½ZiÀ:
²p*4‡@"EÑ4O?ýTç4?ª­ƒö?ž%.§w§?õ-ÑD*Ò<@SÖK¦¿äWLíï\D?ìÛÊ`áÂ'¿Òé,êCÖ¿ß4<Kµ¶¿ÜÔ–j:¿Î¿r[½OTHERpwn3FGL J1838.9-0646HESS J1837-069?¾"W:p½ç?·§0Þ©>‹?h!ó˜#£Ò?móÙ0e"?ìS%Ä ?·ñF*ª´ñ?Лڇ p?ÌL|züÒ?ø7Eò?¡Ù:mŽë?ç:1à.³?Ìg±> Ô?Èͅ"â?­Ç(n%E)?¨*~2­¦ú?•Ñ_†?èIöÛÕ˜?¯å·sV‹›?ŘžDõd?°èww?¡Q$·ZlT?'ÿÉ^u?餇Œùâ?²¿ÕØÜC4FGL J1839.4-0553?צ$N`W¦¿›8g®´À7Eõ­–§À9T'œýÒ(@c;'PŸÖ@Ð:?–îÄ?¯RSÈ)$?ՖBÚ¶@(dÀ
¡©@Ë#œè-¦¿ØœOAÙ´?¢b`¿ªÇ·¿áÈÖ"‹ñ¿å¼žK°»¿ì'ê@%4¿ïÿôým~‰OTHERunk3FGL J1839.3-0552NVSS J183922-055321?É+zOç'?ԃU]¬s?â'MwÆE?ÒanV)6®?Îr|¯ÐÿY?ÉòsDJ%?y3äڎ®»?Š /Bmà›?å¤IØ}l?Ìë)¾²R?ÔRJäÊm?̟ÈGfC?•·®•0Ã?"ÔgÌeÀ?é}"¿å?±Rø2É?ÆVøÃ-ŏ?°´y(/¸K?+I €c?#O=WqG.?Ò¡C
øRh?·Ú¼?æ­¥…óTÄ?·ÙP9Ë4FGL J1840.0-0341¿ïêIò‰Â.?ëXéÀ9iS$jB"À;?Ú˓é@ŸAЄè2@Š…) ?ÌÖßuEý:?êù¬ÿ§ël@Œý©äj@'bˆ‹T\¿Öüz$r뿧Š
¿Ó‹‰ þé¿å»;u!M¿ïúøÞ£¿ïÍQ!ZÛOTHERspp2FGL J1839.7-0334cSNR G028.8+01.5?vû.E?"µtî·h?ޗâ¦ÇÄc?È°éh?à3® äD]?ÇúÚ¸h÷?ŽbB\GmZ?•}uي?چE¥òf;?Îóå@« ‰?âCT#•¯.?Îß$Dò%y?³O4v«vØ?8'¾Ìt?ÙϼÒ8\1?¶PÉeg?à®;c
?µQ¢ èãÝ?…@,%X?rŒè­Eo?䌻¸)À'?¸ú."¿<>?Ö>x}«±?¸ç›‰ˆý4FGL J1840.0-0411¿íÍ
Ãü³^?ã²â`1îåÀ8Ë6Z/ À:¯X¶zzð@§qºGº@Â…îÁê?ÀéÁЈg?ÕTpšœÏ@T´:ç?û£gΛY¿ëDä þè©?îAÔKFOp¿Öç¨ñ%r¿äd˜0
¿ìÿ"=ßßy¿æ°Ë¡ÖªOTHERspp3FGL J1840.1-0412SNR G027.8+00.6?‰aÁçbR?±'Ö=X?âË#WGh-?ÈSþ	¼Ü«?Ùa#5R¹€?ÈV¬¨
?‰#‹GB‡	?"*%"Ïø?Ù&—m©‡?ÉYרּ21?ão‡,!?ÉO½z,5ä?²¶¡Ï±_L?ª|f¨Úð?ב!8F{?²a=ñ¬F?áà›)ú°Ù?±Š+
œø´?ŽöÆ¢µ–?saٖMql?ӗ¹†¥C³?±¬¥Ò¸"?å¸H""‡Î?±ÇÚÍÀžò4FGL J1840.8-0453e¿ã܈.b>?¿¹Ÿ'À7Y…tH§9À9'$~d@ˆ¾)pçŸ@úh±šA_?³uÏ:p`?Ð4°@¥¾@	G{À?ütXåIpa?îfKŽs˪¿ËOøæ±${¿áç—Sn¿çá}ÿ	_û¿é¹Ù«¡¿áĖgµñ¿OTHERspp2FGL J1841.2-0459cKes 73?h§2Š§1ò?c§Zë©é ?¶ªþ³ë"?´Z —"-?íMžÛk?´\ÍšÅ?{¹¬G-
æ?…`ð]3?ÖZ".۟A?Ç¿†u?ä›JÖJ?DzÇj¥t|?£R³k;y?Œpªš"šæ?ϕDñ§Çp?²¦U×ÈôŸ?æåŽ_Zm?³9*ä«d?Q§TdzF¨?CZ!›D"V?–ÅMÐË?«NŽaN»??ëQ{( ©?«~?£uä4FGL J1840.9-0532e¿·@|ûÊ¿Éc\ɯŒÀ6ÁHO$*'À9¢ö{@!À¤¿:¾?ÿžá¢FçE?¢qNCQZÞ?~¢¨¿"?Þóå÷1?þ8=ägF?çÞ&'dA¿¹j"Þ|L­¿ÛO
*á¿ààÙÿ»6¢¿ãäkß÷÷É¿ÓKA\k»»OTHERPWN3FGL J1840.9-0532eHESS J1841-055?vz´Ws?kû«ˆ^6?BÃæ
T'0?E¹·™žD?ïÎZÛd.?ml!,ÁÐe?Ÿq#¦nþ? ÿèó¢h?­QH+.P?²FîX_?í/fã£?µî÷Ú
?®Ëè°fP?—9'µ–"^?¢$‹±ƒžP?ˆR÷+X?ìðø¹æÿ·?œ'ô&-2Ò?"ÎhòZ-?‰'òH3
'?¬}še"%?›,-}ß 3?푳ìÅ?žûž!-ƒä4FGL J1842.2-0751?ï(R¿•²¿ø֍
?#À9m‹U38<À:í‹ÿ}#@an"B€@]™`Ž¶?ÐL]їb?Öļµ'•?ý*áU
È?û¢£h¥Zî¿ïúHÿÏ?ïÏف¼O¿»³¦
@JÉ¿åÛêaˆ0;¿ìXG¢'v¿ÇF£¨f;OTHERsppSNR G025.1-02.3	?«Ov¶b?£û‰`iÖC?š$òW:ðÂ?—²' {Â?í}Cuåm?ªñg'¾9?½n™?£?´¥ÇÖ²)?²
eï_Z?³Þ¯ô¸?êš 2A?»r˛/±?ÁnrUè?´Žö§,?ÅïR±ñZ_?¥'ûKnµë?æ<OÌ'î?§¨ˆH¨¸?Ä`q÷Tc?§¯ÃîÊ1?½
íñ7¦?§»Ž&Ú³?çF£;"ò?²F׳ö'Ð4FGL J1842.5-0359c¿ïÚ¢ÄPâ?Ãå>]³ºWÀ8
°Úþ¾·À9Ÿ»	Uê@Ýp3Ü@jZaueÞ?ÄèÀHZå?؅ZZna@\äŒ×ê@‰Ö€TÏ?åi¹×ý'w¿á<Ó$Õ¢^¿å€™¸£J¿ê?*b{ö¿ïþmž"ÿQ?ït4à‡iÁOTHERunk3FGL J1843.0-0359cNVSS J184240-035858<?²Š°¥"`æ?ĜA£ä?•`òå-Ã+?—ˆè€¼'§?í¢T$%Ê?ÄӋc°·?¦+ƒÇ·â?°¨¼3`?»Ú¹IU\?¼Ëm÷uÕ?ë"l[]7?ÀãÛiȪ¡?¸…ÛÆçnj?ž/pCÕL?È9óìOÐ?©+;0,	Þ?æàþÊ'ó?­à:[Çö¬?i±Vç*ä'?`¶u~sº?­XéÀ1ùf?œ¥oá,ã[?îÀ
µ…?žeTrÙ¯4FGL J1844.4-0306¿Ý‹ù÷
9?À0¸@¸À7±Ÿ°4ÒÀ9zh»«<Y@KŸÅÒ=@K9âyÝ<?¼@|ÇÑ»I?ԗ?a¿¸'@7?tN†@k%ПX?ï%)œ±|¿â0öýø¾Ã¿å'0^—ÿ¿ê–—†™ã¿íïßáÒmv¿ïöÁ'ÜæöOTHERunk1FGL J1844.3-0309cNVSS J184431-030716?s'©T»¤&?mÏÌ»
æ\?ÏXÊ°?Åýõ#¸?èzÒܱ?Æ0>XØ?‡°P=•Ô?+~""šQ?Ñ[O>AÄ?Ä8ÒÂs™?æó— ÂG?Ä$mdö4l?¢Q3IԌ?Ž2^ª«¸?ݞM€ØF³?½¾°üÙM?àǼ_?\?½E<Å!?@2»ÂJ$=?3Œeފµ?ÂÈpׂ'?©®¥a&›G?ëI×.å–?©¹üœêƒ4FGL J1845.8-0831?í"c)›ýÀH㞠jÀ9ƒºéuzÀ;RALÑiê@#ï{M~@©"˜€•?Á"©…JV?Öå-a4l@PÔ~qõç@û†°ð?ïöׂˆ[¿â±Âëc'¿Ýt^ÁVw¿åÞ¯îo´Ä¿êîU'ÙŒ¿ïú–ŸVOTHERspp1FGL J1846.0-0831SNR G025.1-02.3?·€@ׇ6˜?¨´L×Á?ĦÜbQÜ?¹F¿¹˜?çæríö"·?½È¦ZHz?·
›Š?¸ƒ›àŠË?±¡)ÃÂ?¯cU¸¾EÜ?éG- ÃÜ?½ÉìŒöp?Åhª¥6ß?¥‡PI|÷¡?΁À°¢'º?©3ÊÒdTi?㵩.™?®üGé?Æi6K¬ó½?§J÷®Ãݲ?Ààݸ<77?¤fNˑ_?æ-zÿµC?³?ý:)Xi4FGL J1846.9-0227?ØLÎ/d¿½
ò[ýËÀ8ï͂Õ2À9¥rE—¹Æ@BAê04ü@R+Ù¢ž%?ÁƑIhÿž?Ó'mb*W@Á"tŸ@ŠÒÒË?¬ÄÉ¿Òu`Õ,î¿Ú-³Âd¾ñ¿èëð«Ï¿ëîÈáÉ¿ëW€OE¸qOTHERunk1FGL J1846.8-0233cTXS 1844-025?eŠh×Ôۋ?_š>Qîéx?½w«Hå2?¾èí"P»e?ì;ƒá¿~?¿Ns¯¿?'ÞRƒ•O?–|ÐW>?Âя‹rš?·¥Ii_?êêi®?·¥L	G¦x?¤qC½,ѹ?†!xlúª"?Õ~à‹Ýî+?µå!Œ‰÷?ãù{~>;Ï?µM,õÇH¨?XϹRýÂX?J¶–hdý?·$—7pr×? ŸvaTk?í<hrÅ? ¹ré€Xb4FGL J1848.6-0202c?éø(¨E€¿ÔQlĤ_EÀ8RW˜mI¯À9¤mvûßà@ôüî@ç¶ãV|?Êk¿m"¬?ל;À•G@TUêî @z˜v. ¿íœ"N‰{?ï-ÇW嚿Ú<ßï¿@¿êh{œ"÷¿é5BEî¿ïÿ*±0OTHERunkNVSS J184840-020408<?w@ä¢:œ;?‡x¡O«4y?"mLê†y¿?¢+ÚÌ ¶þ?ï.ÏgVù?¥çñòÞ ?º/ç°X?¡<2·A?Ëó§eÉ
?ÆrxÐís?èhü§P:?ÅÖíªuqÆ?¬}Œ~‰Ý?/Q"+?Ãçg‰þ…?¢mD†[›‹?é>T"¸p?£ÍV(¥²,?uášÃ¬"Ÿ?hŸjÝ>?´Ò«'Ç;?¢êÚτv?í9çXÆÏ?£"Ò:»4FGL J1848.7-0129?ïÅP«'é￸}P·
HÀ8'ØÚø	À:S‰X@úFô±e@ND¬{?½©O€W–?á1Ú£O%@"]Ç5ï¦?ûøýlÒ¼%¿Þ›C<뙿ÛwŒ>] ¿ÓQGpĎ¿âgšþôgF¿ïü¸Lã¢?æ®&ïXOTHERglc0FGL J1848.6-0138GLIMPSE C01?›,0	Ôa?¶12Pki?é›9mœ¼Q?ÅêSó×?Æ1´Ã‹Ô2?Â8-Î1.:?"á}ð¨'t?"k=†tQ,?æ'ßÀ{‰R?È
—ìYè?ÒS4ƒ©I?ÇÑ pð7?œ'lñVY?-©Ÿ<`-?ç10CãÙ?±clñƒ¨Ÿ?Ï»¢Òpö?°'-œ€M?N¡'×>Z?@a¾‰tÎ?Ô%‰ÉzF?ÀOAnWÑ?åå'×¢'&?ÀSR4FGL J1849.4-0056?ìڊLl¹?'|[p>+ŠÀ7€3)'°À9¥€(¯K³@£‰™o@-"œ)–Ò?® è?Â&ÕøÎ]@—»s5@|s³Öܛ?ђ'ýîØ»?ì›Âhż¿àKH¾4Ù|¿ä'É oâ¿ç~þþx@ƒ¿êKý>¯"+OTHERsnr3FGL J1849.4-00573C 391?‡9NGOð?‡åÄãT?ªqrkÞÒô?®ø^ß]@?íú«ôõ'?°¢cî`?"0úÂÝ¥?–®£N.>?×Ãñh…¯?ÊÞ¶B>B{?ãyýÃç"?ʹM59?­v`3<÷?–¥Þ¬òT?»+#€â8?¢zöp´V?êÃ9ÚL¯é?§LÚ9½ãè?	̃È$È?lÁä_¬Úf?Áå'ÑîÖ6?«š‰¯ŸÜ?ëH‡²|º(?¬{V
(¬4FGL J1850.3-0031?ã»®¿rä{_ßÉÀ8Ú¬è*÷À:A
±3ê@¤WZn@g8¥Ì®?ÈÔÌ`it?ßÅi`ì©â@'ã'÷Ó@'Ź2;<¿çHGä¿áx{Â=ä¿Ûí$S†¿é_þ"/T׿ü¾, ¿ïõEâb`GOTHERspp3FGL J1850.5-0024SNR G032.4+00.1?möÿ_øU?fMª¥Å?¤ùÞ(¾Î?££»#×·[?î¡Ic
?¤_Dˆ`@?œG
Q(îï?› ʛ­å?¼Ø‡>‡d*?¹¢²Ÿ'3?낶­¥Ì?»$žbF?­µ1¬Õ‰%?ˆÒºïxD§?ÉÑËd'ëf?ªÙql?ç°:(¬"?«˜dWÊÚý?'g"do8_?r:±ÎÑ?³C$ܙ…t?¢qJØó?íMþÚÛp?£»æÒ:Rü4FGL J1851.8-0007c?¼ÿÝRMw$¿Ã·—†nïwÀ8yN»NöÀ9ß:~_@UE®
@¥¦½n‹?Ð?'}rq?ƛi÷?'@hýAߞa?ø´ý먰
?ìûi,êCÖ¿çÈâ\¿ãÑ.~§¿ë5*Ø>¿éSÕj*@¿ïÍ;]ÎOTHERsppSNR G032.8-00.1<?ƒËŠA?%"‡~Ì?€ý¯‹Û?‡·1Nï?ïpµ—˜=‹?]Zˆ©? "N0rt×?¡'–®³?¥Ú, þ©?©÷rb?íšZè÷Ç?®ZÉûë†?¹íq« ód?œÏÄ1Új'?½Í aAèD?¢
PNehE?é­¾c¤‹?¦åš©r Ò?w[ëK\,W?eúÁÆzˆ?œðõm×[?‡¿€×Îoå?îéÀ}úŒÎ?Š"¾à›ó4FGL J1852.4+0037e¿âz+ÙçVU?²¾vrÍýÏÀ7*'U¯^þÀ9n@V1dý@Ë£Œ·ˆî@XçW'Ž
?³uÃ?t#?Ƕ›Ø'@¹DŽO¹@&;Á!Gù?ïƒ9L¿ÚFÿøš¿á>f7l}Ø¿éâŽÕñ9¿ç֔–ûY¨¿ì‡{‰äðOTHERspp2FGL J1852.7+0047cKes 79?r¼òólê®?jÜ6Jìö?l1¾Hšk?h§Ý¨Ïæl?ï¾T[Ќ?uÁõ‹Ÿ÷Î?"=!ÖZB>?–,÷
ú½?'ïm¦?¼3ÞÂљø?깛Äj?¼±6¬þ¤?¹Ø[è{u?¢?3ˆžI?¾žf¶ø­0?¢ªe|î?èñ'¬{¸?¨Ìâ£ðšm?vIë12ØO?l`»S÷Å?¦qgJܑq?˜g+|Š©?îlU´ïÑ9?›GåyN1j4FGL J1855.1-2243?î¦i¤g¦À%цÛPôÀ:f	{¸À<C{cM­2@p¾†¸ìE@Èêí+?ÅGmgaŽ?ÙÆüÿ¦@ ü ÏîÀ?èÍ®z§?ïÑGP ©Ä¿Ü´'drñ9¿ÜÊ1ç٘¿àÿà?Æ>"¿ìAÿ~Ñ¿ïÝv¾"eOTHERglc3FGL J1855.1-2243NGC 6717?ÉÅÌûL@?¾¢ÌwP–?ß{ïdcàl?ÇtJÜ2I5?Ó¡Pµys?ÃéóU"p?½Zn­÷?Ãñ?õGoÈ?àäB@?Ñ$Òñ¤?Öá@àXÜ?Οùã²N?ÍÇ|Û¨¼?°Ò,Feï?àv"?·Éäö?Ð/ý"#á?«áÕey·b?µâÈ­wb?"á'íÖ4?ägy5ƒZè?±ËB`±ƒ¹?ÑéÔâÍìX?¯çAã4FGL J1855.9+0121e¿ïÚg·k³û¿ØÕ[½•øÀ5pfB
gÀ8¡%µ¿j@	-%R@ê쑎2?™=#¡ð«#?ÎÝöjÕâ@8oÏå†6@
Çf,"ÃI?ïÀ°^×ü¬¿¨šÜ æ{0¿ã^ FÇe¿å׈b9°ü¿ëS€™¿êP="OTHERSNR3FGL J1855.9+0121eW 44?¥+
Ó5?¬'PÌ¡K?è@˜g·?΃¿o-Õ?Ê­üÓ "W?Ë`øP§Ô;?qÌ·ŽÑ×?…Oª#@ýå?ë\¹xê"í?ÈÇ^¸T?Áþ´_奾?Ç¡™ÞÍðÔ?¶'4:‡õ?ªé}ÿ†O?ßY>:Â<?¼ƒÂE´žk?ÛiÙ³#]Æ?¼jŠg>>°ýv¡µ>¹Òm¤uÖ?âTQëß¼x?ŧz֛e'?ÛWX"A)?ŧx<ìÐ4FGL J1856.2+0749¿íª¯ˆ9Ê@ö>e–\ÎÀ8v(]íÀ:3ùÄ|œ3@&#«UÚ@(îñºÂß?Ù¥"Ò?Ò^zښ@{ؾr–ö@á
s(?â¿âT'nâlq¿ê3âààU¿å8Yã¡$¨¿îa¡Û‡{¿ïÿCÂw‰NOTHERunk3FGL J1855.6+0753NVSS J185612+075340?¦NúÚW–?¢$·ˆ
Í,?ڋï؞J?Îä"â:GØ?áUføâ?Σ£à ;?±S\C?±zOCJ?ÜêۖdJÁ?͛s‡Ÿ!?ÞÔbÔÛ^-?̪ð°äÃ?½b¤8°À?¡1֊?Є€Ð¿/?¯LéÍdž?äk9Rg?°A¿©¦Üí?ƒ»»xþB?nÞçË¥þ?È6|cáËà?¬L™rd?é£qù#"ÿ?¬©xǗbD4FGL J1857.6+0212¿àü¡ž¿ØÛaåùÀ7••žÀ9oAÿ~ÐÀ@p7ÿÛ=@7ïZ–O?¸#¾5y?Ö½"થ0@ ¼cñA \?úv8kX?ïʙ쥰¿ß4È<V¿âùÁÍjW¿éöå¿âÙ¿ïÌn"rp¶¿ïЌ­OTHERspp2FGL J1857.6+0211SNR G035.6-00.4?Ž›I}j?¯ÓÞº‡Ó?Øɘ‡Ž|?Ï®yTD?ã Çl+×M?Ð&tÿþŸ½?{IƒrÈ^î?"¨s&|?ããÞ:"ñ?Ëñ¼ªÕ¹Œ?×Ë}îü~?ËÀ¡\/G?—Û(G—`?Ša†µ$|õ?ãC—ƒ_U?¹~ƒeñi?×ûtÐà?¸Ðáç›Í?ik]Ó÷?t'ªš®)?Ðûköa?¶K" §y?çf¹wC	?¶L|Ò`Ã4FGL J1857.7+0246e¿h¸.B#49¿Âÿƒ
6À7ô'|À9¡v¯‰Æ@ ê¿É.1Â@ü,9
ä?§!\=ú×?h'"èl?È2<Tì?ý‹ÐÓŠT¿ïàsÞ-è?ïÿàU?Íu¿æ=^ä'å¿å'$óÅ¿à™[á}3¿×²í'¶'OTHERPWNHESS J1857+026?°'q5?Æ?yUiÌ?U.NâÈOÓ?x‰+°+b²?íå&F€u5?ƪ>Ë>?·'PB'¹?º­Ð6ÙÇ?°+/¿ÇÌ?¼[jÍ¿v5?ëõ¯ÿ¶°?ÃeLj<Bù?¹Àb/0Æ? …£óê=J?²Ô'Ë,?Ÿ£\,«H*?êmc`¹td?¦£Cë®´,?¨+‰"ËÙ1?ž—#lB–È?¥ØÜÂr°?™[aμDB?íÆpA?§†	úx±4FGL J1858.3+0209¿ÞˆSÇ@5¿áu"@òŽ}À8øéëÀ9ûïº7žÓ@!ÅÈC¦@¤ßÎ1PÛ?Ùc²ó?­çÄgB?äÏñå‹	´?û3r@9V
¿ï™L'9«?ë|vÕIs?íœ&¨«¿á1J$ç@¿æóé;˜\ƒ¿ïú 9påOTHERsppSNR G035.6-00.4?ŒÉ¯¸;?Œv­*6è?€Vi{»–?'hçyD«?ïK›Ò1|?™ž¥‰J?®óQë÷g ?³~|ãZ²ê?–¯:Ӂï?£ðǾ?í`Mgiíy?¶cyb'æ0?Áf¬†¶ÿG?¢mÿەc?¸èr0è?¢ TĹx^?è¤ACú?©™/9ÛU?šYni?"Jèâp£?|Žr7æM?ƒÔ+AXr?îòy+¨G¼?˜þ}Xñ"Í4FGL J1900.8+0118¿ê#O»T)x¿÷ìqþJÀ9'J HÀ:HgÒw0¹@òÉÞ/ö"@f?šIÂÂ?Ñ£#=­?Üû=£z@Ͼ¹ä'¼?þïSZ'É¿¡…¡êöÙf¿«ŒÂƎš¿ä¦ˆ*¿ìÁÓ_
+¸¿ìšƒ¿<ÁQ¿ïğá§OOTHERunkNVSS J190146+011301?yÓò
H¦?€xLþ–ã?ž¨—BÀþî?œ|?yxÀ˜?î×aÏgù?ŸÌŠ\ãñ?¯•"´>À?°/]"ž‰L?³2ƒ|M?²ˆˆ£¦öÔ?ë"ÈFR̋?µÏLCÐü'?¶Öa¨V:»?'iQ½‰?Ã¥Lè;ZT?¢jIM?è;àæb?¤†·A"B?xëÉÏÜ<?dAØðªa?³üpnÜOŒ?˜Û¶°R˃?íNš_ôÖV?™h®bçô}4FGL J1902.8+1451¿î.ï¯ÙT£@	&A³)À:l*pìÒÀ;½—Õt;@ cȑª@Œ$ÞܙÉ?ÇÕ{]2?[Ä}Y-T?ª!Þ:ø@|šCã…?îb÷ç,Êc¿ê»ëýê|¿ÜÔ	­þ«¿à@ï´XaÁ¿à'ààUÚ¿çt¨+,ÔOTHERunk1RXS J190249.1+145133?傑$éq?Â÷Êy—Ë?y	˜Z˜?vÿ‰þ)!¿?Ԗ¹ÕT¼?Âç֒«äS?ÛA¥…¦¶?ÆÒr}´–b?ç·WlŠ€?›ýÙ´è^?áçŽ_ÎòÖ?Æf÷ñPC?âÖGÚc?¬ô¬àˆÌ?¡X˓¡-u?…©¨QßÚp?Ø(´pü%‹?«‡©|æU…?á,@IáÒµ?«u›â?…ð8dî­G?t›Zj"þ?Ü÷ý©å-?«r	ùÉG4FGL J1903.8+0531?v'Ùèemç¿ÏPŒŠgwˆÀ8P*|«LJÀ:ešŽŒ@ØéH-–;@Ù7fžšŠ?Àä8yC7ã?ËQäç ¹@ã\[J©@˜/…)?ïkV/Ž?×!¦BõH¿çÄM¢J¿ç5†_*2¿èa.ÿÿe¿ê¹'Ñ!EOTHERsppSNR G039.2-00.3?"É>mþ÷?ŠÞ^'kq?Çãl!K'?ÁU»-7²0?éhØý¹Ë(?ÁÝ¢ºD9?˜ ‹r©ÂO?˜Àk/?¿HèᯥÎ?¶S§.??ëQވ4½4?¶k¹o$tØ?±uì¢kæ—?"†MK$$d?ÃÓü½ÆÏ?¤ì\'ÌP²?é

lƒz?§Ìñé³^4?'kŠ&k!?mXÄ2‰HÊ?¼aÌÄ֏?ž…Záäm?ì"¥Í¹?Ÿ~ý+x644FGL J1906.2+0631¿íG¬uÐx¿ÓVŠüñ}À9½1NV¥À:JNÇä/À@%ž©xß»@˦"c§o?ÔSs¯ûî?å©Ë@Ó@;ŽK‡½Ï?þ‡ýÈI¿Æ(!\F'¿ë¾aÔU¿ØÈç$'Ú³¿í!Äuæ6¿ïÿø="ßE?ïÿ /ÄêOTHERsppSNR G040.5-00.5?³eDøÁC?µ"¯ßÔ̪?«°2gxq?²pØ$gpn?ëØT:pWç?À2
4H+^?¶¬˜X¥€$?À؅6÷$"?³ì<}¨¤¨?·ù''g?ê¬åe6;h?ÃL%Í΂?ÂBzP­À…?¢Rdg[©?ƘÍQ
?£êڜqPy?åÉ.$@Lž?©,âs²?€êÄÌ~²?r¡¯þFÜ?² $ˆ±?¢Eø™Ô?í}|P[ʐ?£B€Ðæ4-4FGL J1907.6+0703¿ïC
Ô²|ó¿ÖÑ#^))À8Õi´Ï€À:ÿ¼ä!}@!L/å¾@—ºÇç‹?÷ØÎbÏ1?»LemaØ?øæbÕ¸-Ù@<‰Ên£¢¿ïÿÆ¿l'ú?ïÿþR€ÖT¿ê¢ç@k€¿æ¶a@aÄì¿é0Ձ¥‡¿ß7Cõ"VOTHERsnr3C 397?­ãÃßó?À–ýiSý ?Èw^cÊ_H?έ®Bv?èözÏvÿ?Ыnf¢YË?§rá·½U?´4,&	á‹?µû}g2?À¹eæ?ëÉnWê?ÁÜg‡aÇ'?¿¢³Úß#Ì?¢™<‹ý?ÂPHaäE?¬h¼uÞs?çw—l+õ?¯;p3ÿ[?°°=Ïз
?²DopãWe?tÂ{æ©?jÅ49F»?íÀsN9âø?²¨žCz4FGL J1908.6+0915e?äñ(I²?ۆAãz8UÀ8='ùCM]À9ÿ_tڝp@ IË%,à@$Hdà?àë¤Éx"v?Ҁ3â/µz@¼`ˆÖÓ·?ýCƒÃ˜þ?ïÒ7y…¿ádƒ7W…"¿äLg¢%¯<¿æ¢_I¿é ÃÄæN?­[ƒIBŒOTHERsppSNR G042.8+00.6?›T›S¦?¥vøñÃZ?ȑ—àøN?È£ú€1<h?éûµ-$½?É.934O?šqšjí_
?Ÿú€/ó?Â'îly?ÂÐúg
ä?ê¤Î§,ùê?²YgÁu?µïj‡a?"äæFYSÈ?ÇòíÀÞ j?«÷ÅÇÎ?çb¡ñÛ&ú?®[­#º«¯?">?ab?pŒæ狍?¤-¡Ã€1"?£µzýb?îjäêÊw_?£ÿ©6ñ4FGL J1910.8+2856¿Ò	*\[1@!ͦÅÒÈÀ:_:Ôd¬À<H>¼(@!w×Å#`,?ú+RÿTÿ?ÅÛìdí•o?Áq¤ƒ³ÿ?û°^òԞR@©…—Ùûß?ïøøo"¿í¦÷P.½?ÏI5¾}ԗ¿Ôÿ©ƒq¿×kr¿»l¿Õ/â{ŠºÚOTHERunk3FGL J1910.8+2855NVSS J191052+285621?èƒ"Ž!²|?¿X§ËG;h?bÐF[A¸?\ßmýi?²?ͨ4®ù?¿6¿oÊÆÊ?ç}¬ÇØÃ?Ç&	ÅÖ?aYO­X?r÷Ytú"'?ÑÐRGÈ?Æþ†Ã¯¸Ñ?êØî¢V+?¦}÷]Ô?í?{ûÇ:ªª?hïÎ!.x?ÃÃ¥™LÒ?¥ï·­;J—?í+ ¸ùÃÚ?"Íªpì?fQ7èŒ,?Uœo¦ôP›?µôpxíÍ?".ÿW—q4FGL J1910.8-6001¿î‹JáЕÀ9¢È:£jÀ:UàñFÿ™À<¸6<Òï@/H—H†'?ÿÍÃ7!Õ=?Á¯þµÓ?àݰʹ@œb^™éK?÷Ø腏÷?ïôºâ"Š;?Û:`¤¬¿ÞI
DâG¿å¾å¹,ÜØ¿ð?ïŸJžê	OTHERglc3FGL J1910.7-6000NGC 6752?ÆìÚ¸-Ù?ŠÀ	Ù6?é)×ï—ê?ÄÃ
ÖlàX?¡¯& žÅ?¡ÀÀ.Ǿ?ºzK+?»Æ
£ícË?éٝY7?Ãα›Gk«?·)Ê0Es?¶vS"U•r?µ C­7?¡4,Ñú­0?éuúòÄ_›?¨×»0åO?¿/ä¼Éôð? 2Ô]ñ?À&f'q–?§{ÈÒª@?歅¨NÝÎ?¸*_[Jœ3?Å,ÂøB2?°TºŸùE4FGL J1911.0+0905?çÔ Û¹l¿ÆŠæ¸Ü*
À6¦»¡+^SÀ9©\¥"›@ \Y(eNä@þš9҉¥?œŽ÷Õ9Õ?¾f{µ*Ó@#,Ùb…U@Y–8¼?ä²Àü§†?ì@֟^'¿àó\îî_Å¿âYöKKWí¿æ•V©Zý¿ã\νgÔûOTHERsnr3FGL J1910.9+0906W 49B?…ό佃?€XԚ!ñÙ?²]pÁô8í?¾¥*/3
?í]´1ií?¾®¥£H5?'ðÍȂ%ù?¨Q®Ðžó?ãAqŠÕ‹Ó?ÑÀ‰Ôˆ?Ø^
ÌÅú?ÑDNv	??¨4øLé?–Ôد»?»˜£$%Ùµ?¤òO£?ë	«;özë?©MÙÎ81¿?O®¥ð€Ýp?>ˈ`•±?߉_dó?¸Z‡`'÷?àhO¦ÑfE?¸YŠ×Ba64FGL J1911.7+1014c?íèKgvJ¤?ʑb}ù€	À9"¤ÏWÁˆÀ:C_?*¸:@öÐÑê@ÖÐ& û?ÓéLçvÇ?ÛÊދ?@
¨d©ÍÄ@z|rí2?¹¨w­áz.¿ärÑCT§¿çò›Þ˜QE¿çè§ü2ì¿ïÿàè@?ïí—䱛OTHERunkNVSS J191157+1007208?ÉFsjáñ³?ÂÐûØv•?²á,&Õ7ò?²RdŒª?çR= lܕ?Æng¿
sg?¾ÇC‡1õ?À&N¦§4±?²v#Ü ¶?¸é—"¤âV?éØSˆ—‹?ÃdS̗sù?ÄYLüm³Ë?¦}I¦ýÉ"?Ħ"Çï'?£Œ½G˜S?åÀ$èÐ?­¯KK/¸g?šKŸiÊ}¬?‹ŽV@N>Û?¢Õ98$ëÊ?"|\Ð+ã?îOq/]T?›˜:Ó!4FGL J1914.5+1107c?º¸×âÕwÁ?r;éàåЭÀ8þ~Ä+=›À:mܺ€™î@Ú¹w/Œ`@¯P]¥?Ëô²YƒÿÔ?ØN»{ì‹@D7£~ö?úi#͏•_?ï¢á ÁÁ¿ëtŸ¢G¿âñ—‡p¢¿å߂ç¦lç¿ïêX~FVü¿ïu üÏÊOTHERunkIRAS 19117+1107%? ·â´K?š:
;ð­É?Á+5Ú½Ë?¼ÑQFRà?ê©ÎTiG?¿f¥dLÎ?šOÀ–'ä?™ûí3ž.*?»Hg=u¨?µ­á>ÁÇQ?ëÆÀšL–n?µ±ÚJÕå?´ Ü†ï5?"u'	±Ú·?Ð)5Ëy×,?°;¸>£?åWI‰e$C?°rË2ƒ}?r"èºë?]5ô·ƒ–ˆ?Á»
~Zâ¹?¥£‡f¥?ëm_uÞ?¥Ðϱà;Ë4FGL J1916.3+1108¿½Y ´"Æ=¿×ã	
¦¢À8hjª˜Å^À:#ˆY@û®a§»@$,<žìÀ?Â}BJþ+?Ï©ãhőD@€aº/;@£ -²k¿æprÄBº?ïÎ<~`ƒ#¿äyh6J>è¿ê×0h}—Û¿ì/#¿!é_¿æ=\aª¿ÝOTHERspp3FGL J1915.9+1112SNR G045.7-00.4?'»b´^h!?ŠÖƒbîQˆ?Â,fzpÿP?¾½Ò½Ò³?êßKÀÌë?¿ÉpZfµß?š5WÞÀØ©?™éôˆÈn?ËW.šúÈ?Â>Þ֐v¢?èX"µc:‰?Â	Ãå@'?±7@¸?';Ž¬ÁC	?ÌÛTáó4?®Ü}`ô9Ó?æ§ÊòŸ'¼?¯^ÏÖYï?‹ˆ"Q?upÇR'(b?Á'¾[¼Œ?¥}s:
¤?ë-/ßg™?¦&xd•4FGL J1917.0+2245?ì0g>'­ï@v®b~zYÀ:Rß&k¤"À;›%d=—:@îƉ;Ók@"%kÊSv?ƇE¯Ç?Š²?‹cÔn?Í©Ä_Z@ÁÛÍEÄ?ïÇSó¿ãt;Áw.5¿ì¶À5¯å¿ØýŸ˜¿ák¬N"r¿ïÿï0l¯OTHERunk1RXS J191710.2+224852?âï°+¬S>?ÈÐÇ+€\?qÌeÕy¾?j'ûïÞÌ?ÙÙn`ž?È
dÉP~?ä¹²P"­6?Æ0çÜL?s)À!ø§?…î&õuí‡?Ö?ô^T¡²?Ś>ü	
?ãS)ÍZÃ?µOQËlŽ? ÉkV‡?ŠRyªM:?×YsB½sª?´?§iÚb?èÀÒ½0"©?ªwzÉ+!ï?€msQG?nk'µ•¦?Ëûþ4›x?ª>W$—»-4FGL J1918.0+0331?Ãö
uq=§À-ÕM¤ÎÀ:Tâó¾ýÀ<jì$·@"*ÂsW‹?øé¥e¶š?Ècêá	ðš?Èî ÝÓN@B='1Æ@Ýw"áú?ïÄ:Âs­w¿ë
Шú_­¿Çè´ÊL"Ù¿Émêi?à¿Ò€XÀ`'Í¿Ü'kÏOOTHERunkNVSS J191803+033032?á"ÜS̞`?Åf]WÚFf?sIëz?hŠ%@yµ?܉#@+W?Åa›IdµÕ?ߤ¸¦_†	?ƞ
°ƒ€d?aLRë˜Z?qæƒqi—?àœ`}Qb?ƀa@'ê…?çëf ßÞ?°~Ž'ŠJ§?Ž,˛Hˆz?{H7÷ wA?Îq«Ç÷þ?¯erÔi¼»?ç­ã¤b?¬¿€æK?ve¦ÚT?i6N1$Ø?Ñsævù?¬Êä7]Ž4FGL J1918.1+1215c¿îúd×ðí¿Ð?ºà¼ôÀ8½3€`°À:HKjaž@!"å]<@¶"}æO?ÊJ¯;At"?ÝЌÀ\¾@±JÓbé@ ,|_Ìï¿àÓí½Þ€¿âzüö`D¿ä'§èM‡¿ílzFíû¿ïúÍ%¸ m?ïGnß0҆OTHERsppSNR G046.8-00.3-?Ð_¼??š7@äŶ?¥-ÊNá~?²«ò}Ш?í¾¬
¥/ï?´‰]ö…?²=h?¹µ5F:û—?¿9Ýü¤­?ÀEŽ^Á ?éÕü±n‹(?Ä­‰óVP?¸ÐÓ¼‰ Z?œŸÏ%2W?Í.o üÊ|?°$Ôn¹?åšIÀ/™W?±wú?㸡?'BÍéïfß?sPŒƒoÇ?´Jl¢x?¡Í—J(v?í-¡׎?¢¢(ÒqXó4FGL J1920.8+0418¿èzžk²ÍêÀ>ˆXÿu—À9¨" [TºÀ;"×I''?@wì…#ëÃ@]ô!¥l6?ÍM›ê+ØK?ѳ]û]ÙÐ@7ã#Pg!?ý·ö|b?î€m®YD??ÛobäPÌ÷¿ÛÏ|'l+¿ãÿÜđ•¿ë	FОé¿ïÿ n4'OTHERunkTXS 1918+042?°²cbÀ?¡óŠ"+.Ö?¡G¶èŠ"?œ(x­8?ìØÏ9su?©$ênc0}?À<SIíž?µ@à½ÒD>?³¶üuÿ³P?³tËдã?ézžøÎ/?½§ˆ*‰Öê?̺tž¼Þ?¨éè›m­¥?Ä
þÄaB¸?¢` 4|©?ãÍã'8wÒ?­6Ã"?Ê)"•ƒ?£îôT?ÃÒP…=1?§öˆþ™?ä†!yÓOì?¯†ÊäU–þ4FGL J1920.9+1408?ÄRßF|L?¢åŽå‹ŠÀ7ü֋'oÚÀ9¹°xÙ/²@µgJ0@'³Ù¶À?Ãe7'>?ÏxJAÃ@§~^ª°?õÉå"nâa¿×ÏVˁ?ïœ}^Ðoï¿èÉ5~'ñ¿é&$ÂW(¿ï9Ä6%¿å‹‰ $¸œOTHERunk2MASS J19210164+141003?€ôa Τ?'aí`y-?ɏmµ~[Å?ɧ_ֈ8‰?é ÁåÔ?Ê+©‹}Ŭ?'(iO®Pý?ˆáï"ÇÆý?à˘äª\?ËN²Göä?Ý׊ì-Õ;?Ê®êiüaË?²‰ˆÛo?•|pØ.te?Í?
ë.û?®‡è¸V?æoÇËiÂ3?°Zv°üÎ?VI€ {mU?C|n4X´"?Óx
q=&j?´Ð˜Âqâ?æ8Ö/?´ÕJ}ß^è4FGL J1923.2+1408e?Ú)hèÛî¿ÝŠâ²_¤À5âœáL¶'À9t3poÔ¤@:'-ºM@Z}Sèµ?'d—·Ë?»V%¦'¶(@'•Râûã@É¡
&I–?ïåæä¦f¿ÌŽ¢…%™B¿á'r½Œ¾¿â'¿Asè°¿æ²*ŠF¿å[1Ÿ4c4OTHERSNR3FGL J1923.2+1408eW 51C? l+ÄÚá²?ŸÇJ
̂?r]úÌGBB?{š÷ê7v?îԁNÃa?¡™âP;L? Â'e¯%?¶šQŠù?âé¿V&]º?Ó+«±"çi?Ø1ý_Û?ј¤y]]Ú?Ɔ«rw6š?³LˊÏî'?µÓҁîk? é"Áå§×?ç½z©ôŒ?¶Ñjµc?WGÃÄÇß3?K֖Rò(?Õ
·rI?¹¯ ãï¡?åodù?¹¶"V¾{G4FGL J1925.1+1707¿½øpKŽì?á†e_UPÀ9!<MŽ(LÀ:"*—ƒ>ä@ Úº¶ö@®÷ÝÏi?ó"»äG=?Æ꛿¹"à@®Ñ9C?òÕO[2¿ë"²Dx«?ïú|"eZ£¿ää­ßKÕl¿ç–Pn­\Å¿êäÞÚ4"¿æZêg‡OTHERunkMG2 J192501+1727?²òr {&÷?®¹èZßè?Û7"c.¼?Ðgs2¡'?àïŠYŽD?Ïp¥'Š
Y?£7Ú;ðµ<?¬xñªÔ¡~?Çøw/>ð?ʃiÃÛº?èÎdqs0?Ês'§ÞN?¼—;N¥?›€'£ET?Ƙƒ(ÜÒ?«oLîc?æÆÿ47ö?®vC¼%/ã?ªº}C5ù?¦<÷´…=z?¥"Âvý?µ½Çhä?í
$Nߥ1?¸º#Â2œ;4FGL J1925.3+3705?ê	Uži@#™·|¯ÞÀ;CØ>ð֗À<¹šû@ Œ6%«á?ÿ1ž½c£?зObïœ?¹Ÿï^V?ðRtý¾@àDª~ï?ïÿÅbu@¿ã+ÂüirŠ¿â`GÓÔ(¿äG@'‰?È=Qӟ$¿ïþæZ<ŒxOTHERunk1RXS J192520.1+370527?ïüM%? T–Yÿ?@%Ë2'?B•bMoU?›ÌÔiðáº? -:_Îfâ?ä»x˜€?ÎÉÄçŠK³?gFõôûj?pªueì?ÖZ€òæùò?Η{Påú?ëÚÎÈ¢ Á?¡vjCGÀ?|ÙPy&©?sÀêt®?¿[ô¹§g…? ¦‰£ÐÉm?ïØf•;i?ˆ{"Ú
èn??˜.Ú^yW?B3 hç!»?œæ'qïÞ?ˆiKBo†@4FGL J1926.7+3027?ÝRšš@¹èÄzÀ:•ùµc$À<UÛÔ§@xY W¹O@=áâß?Ô.ËÅeÐ>?ç|}T¨@LлnÖw@Ë#ˆÆ7²?ïý± žÛù¿à¬^YQ«¿é!¨üãëͿ웭p3T¿ï÷7ÿöšÑ¿ïôUªV€OTHERsppSNR G065.3+05.7?Ùx~y›È®?ÆÂð'{?Õ²Í^rƒ?ÇvГ[Œ?ÐÔ´(KÄÏ?Âg"›â¨?ÃnXaÈJ?ÂAúÎð}þ?×ïÄSíõ:?ʕœX½Vë?ÞY{. ?ǎz
6?Ùð•˜É?®@#SJ5?ÔQ>Cq.¼?¯/2ÈK'¢?Ѿ,$‹2?ªDøªÆ?À#+°­ü?¾¦Ó§šÍ?àȬÏF¬ã?¶Û'ÆCf?Ö]‰pÏ;?³à‰è%ÜÝ4FGL J1927.5+0154?ޖù]ÆÒÀèp—AÑÀ:Ê]†ÃÔÀ<-/à˜[¬@!ÞÓč¹?÷êSá(¤d?ÓûÒß5…?Í6ðÂuZö?ý[íœP-?@d¾Ö"÷ž¿ïǐÀI‡?ïuEâb`G¿àkbŸ1‰¿»<
rIÉx¿ØmÙ8>¿Ö0Z»¸RlOTHERunkNVSS J192729+015353?éAûX'Mæ?½'w6ÛEœ?jã[+õ¿?`¯aÝ)>?ʌ…1ôJ?½fÙÄÑq¶?ê3eü½?ÄÂl˜ˆú‹?H'\«ãÁ?hì_O©?Ç8a'È?ırì¬?ébpÊ|¸?¨âö¨‹?	Ætl?z™—[ä«·?Èu'*›?¦¹Ô²/?í(ÚÛa–%?"Móž«©?cÐhÅl?[K+¥Þð?¶p©?">1•*94FGL J1928.4+1801c¿î¥±I°ðp?ÒC.=€6À8½ŽwýhÀ:dÍcˁs@Pœ¹ʪ@>¤€}há?˔VúËë?ŀ¬"]M
@[µƒ+ß?þÏðH'2¿ï˜"}?ïÿÍgý?¿êpÓ§²a¿åÇ~)¿îÝ¡0fÐ?Ý»4‰tˆhOTHERunkMG2 J192830+17598?¬¨2LÊ8?¨¦_¡Âj?Ĉ÷ß[€?«3Âc"ð?ézÝ;ˆÌ?Å ÌoÄã?¢°õü œÇ?£dzóœ?Î"ë%°.?È«œ÷Â?çL5ÖÉò(?ÇýŽPq?»ÑÿÕÆËÜ? C+Ä»?ÈñÍ,§z?®ß  çú?æILºGÞ?¯'©ñ´üT? yÇØ"þ?ˆ\´‰áÓÄ?¼Â4q™—Õ?¨wÒL9Ɲ?ë`ôJ¬æ?©"CÚ2D4FGL J1928.8+3126¿âòYàWT@B÷+E((À:g²Û‰þòÀ;ë×!ºdë@Ô]ú@6?<Uñ¤?ÌÖ¬	2ٜ?½FÚ@9U?õŸf²¼€N@ðHäJlá?ïÿâ£Î¦Â¿ÐP¼{Eñ|¿íåmã2ià¿Ë'yꧩ'¿æ"9Pƒ¦¿ïÿ¸8º1OTHERsppSNR G065.3+05.7?ëX$ò?·p	éŸoý?‰Æ$' gq?"­¢Å	0?Â+m¨%eÀ?¶â¿4yæ?áÞP_ð0?ÉûpIÇA?œ¢¯"îç?£üX°?Ü.eÿ²?É!V Í:z?äîà"ë/	?­ËêÂ-£?¦í ¨¡Å?Y	@Yä8?ÓDšá­¶?«qTg|›?èý…uù?§·/ŒJãÒ?¤k%'±9þ?'Ü4\I?Æï ËÍ?¦ÃmúKö4FGL J1929.8+1832¿îFVdvÞ??Ð=çâQï6À9i>‡ûÀ:x¦'@âdc¬Î@µ€šÅÄ?ù.¤"‰—Ä?Óf|`Ρä@`µ$9›,?ößz!8?îÐ^½$¹¿ëç?¿³‰°¿rÜHÚ~*¿çz
½É#˿胦³]þ¿Ôòb~OTHERunk1RXS J193012.1+183201?¹/S'd"ˆ?´›:¿þb?Ê|U€{F ?Êv©·Ú5‰?æ;:ôÇ?Ì
@5kR˜?«{v­r@~?´jUl¿,p?µ·©ø#µ?½Þ¼vîêý?ë'SV'w'?Á£þR¶PÄ?¿J¯8¢œ?ŸÖiï³?Çwğ£q"?¬ö¡Äê?æ8¸÷d?­IÞPÂ??´ë‰?E¿"?¶#ND¨¶ð?š\_ñÏÊ{?²7jFÜ?쏫؈ɼ?½&Fà´µ"4FGL J1934.3+1859¿ÔÞ÷‹Û¿Ýó‡·aÀ8̔<b†ÞÀ:lþÀdß~@s	%˜•ä@¦b…0V	?Éлļ³?Ớua«í@¦Ó0"'@ÖJ¦Ar¼¿Ô€˜›¿äð˜ÿjÙ¾¿ç/æw˜½Ò¿îvþdŠ¿×@Ъ§Þ׿ïÿôa¼2¡OTHERsppSNR G054.4-00.3?Á3mð"Â?¼v~÷¹˜?Óú…C`J?ÉælL™?áµü—â*ª?Ë-å‰ë?©½4j|,?«-Sœ˜›<?·ŒÄ"jRˆ?·×¦ªàzü?ër"&êòí?¹6‡t›Mï?ÁË6ûÂ*§?¤Ý@¸th?γŒÔlÍù?°Züy¬§?ãàOôAØ?².ä0ÇÛÜ?‰A5 Ž?xàŠ:_|?¼íá—Ü?°ZÙ*߁¹?ëýYOLÀ*?°dü՝Ù4FGL J1937.0+3003¿Ì/:­GmÊ@nJ82vuÀ:j´©ÀXÀ;®º××ÂÊ@ÌýÔ+»Æ@ƒπÜ3?Émõ¦à©ù?¼™:Ü?òŸ
纏?õù>ëM@{?ïþœÚñÔ¿Öz€5D…¿èў"•V>¿ì‹©¡¤ý¿ÙLªÓ}Àö¿Þþ®Ç(HOTHERsppSNR G065.2+05.7?ßq¦SŊ÷?ËO'íð?~«LÈGô2?yÖ\_«¯£?à	Ö<Œªœ?ÍøI?Øgq
÷"?È':®ÿ9?¦R'ß	ÇS?«z͏;2?âg`gÁ?ÇD4Š‡÷C?á›AÈn‹?¯àãr±Œú?­ÁÚ¿Ï?'ðå+l)?Ú@™A?°?®¡(>O??ß^n+'4ó?°Jö¼v·?ªê´ÍÜF?™ß£Nƒ?ÝD;:²J¥?°†'æ?^&4FGL J1946.1+2436c¿Ø8"±*.þ¿µê‡a¢v&À9ÖPfIàõÀ;1Cót×B@î«}œ¸Þ@ëø[ÆÐ4?Дr¾8Š`?ÛLÜõ)@¨>]2àþ@ìA‰ã>¿ïÿ…@ò
¤?ïü&âAþþ¿äIE=÷²T¿á‡n¾ú|3¿ïÿú Âî'?ê<—Ëc@AOTHERunkNVGRC J194625.5+243638 ?Õ»+:ÄD?ÁÝðkf?¹p×ç¦Ô?´GÌÕR*?áôOeÊ]£?Ä÷%5xt?ÔVo†"r?Цíݤ"?¹ñ'øýj?Á3@¸˜ë?ⸯÉù?ÐÞÓm§Ã?Ò®ê*ᇮ?­öÏ'à—?ÇVg~®?¨œüôK˜D?àçõP«\|?°¦Î)¿£?Õß×
[¶Ï?´H'À¦Ž¿?³À纻J¾? ^D;hS?â—÷ú»B?¶ºèˆÞÖÏ4FGL J1947.7+2744?ãE Ä2õ?òñBè²ÜaÀ9|Ô4 ½À;)}œ
`@¨MŽ(LO@NU:Ä÷ì?Á¸Û=ÓË?ÐÂi\ƒ@Ö,wWOr@ý%­c¥í?éìjVµï;¿áÛÌ`ëÓ¿Ùp_ùºÂ¿æïÄH™Í¿èGóÐG¿ïÿÈ¢› ÛOTHERpwnPWN G63.7+1.1?ºìÖT÷‰?­ìz·E–d?ÐÖÊüyÇ?À±ºt?ä˜yÏâàk?Â;¶Žk?·‡¤N"Ï??³4à
†ÿ?§_ý›¶Þ"?§5ÈVß?뙜qø/?·ÓR>5g‰?ÎûÄMýK?ªMdœºJ?Ãiyˆ›¨Í?¡¤î}PÆ?ãf°Š"Öz?¬i£µ¹"€?ÁFèƒ4'? aE™î?»uè+ý?ùñü¥Q'?è?'<5øa?©C±;6Â4FGL J1952.8+2924¿ïPç'I>
?ðórS³À9‰"ç¨ñ%À;F"ÈŸ@£@iëw1æ@Hþƒ(?ÉçE³Z?é£opÑ#t@–¼b~?ü¯$¦}ƒ¿ë!ƒÞFqԿـaÉÁ¿Û"Êý¿³à¿ëÊ55kó¿é¥ŠÔø³¿ïüÚ±'ÝãOTHERspp3FGL J1951.6+2926SNR G065.7+01.2?'G@š÷'?xÆtAë?º¥™ßÚ3B?µ4§Û€/?ìb/ÁœM¹?µoVBzM?¬y	D²ß?¦¾S†Ÿ¼?ÏzR¤e'?Êv«püÚ?çP}£Á?Ê»z"w~Ê?À‹þ"|ã;?ž¤&û©¦?Ó¸§"‹Î?²Ÿrß½]?⬘ՁJ?²YzS¼?"PH<Œºì?€¾A&æÏ?Ö4óöÌ+1?º°[E6©£?äCµ"?º´6¥
ö4FGL J1953.6+1846?ïuÅòhâÀ)ùHUÚ'À:7ÁM<ɵÀ;Ë«¢°™@OÔS©Ë@ú37dñ?ÈÈZLQ½?Ҹ϶¤l@	ç™ÅXd?ýbG‹ÿ"?ïÿþÞ÷¿àiÒ+±^²¿ç©.ݎ$¿æ.52ôD¿ïÿõƒ¥;Ž¿å¡»§
›OTHERglcNGC 6838?é9Už›y?¼m¹Á/V?§VÚ¨Vj‰?¢«¯¿yOo?ÅDòÝw÷w?¸ŸwùL?Ê*C¥^Ð?ÁÏAâ}?·ÚãhÃ×5?·b×)i°?æ~Ùþ-f?ř,¿Sgu?ÚÇnÀq?°!øåÏæ{?Æ#´{r?¤`C]Lil?Ú8€Õ³?®£+ær?гI¢Ežƒ?£ùoñ>R<?Ò£Lño‹?­—Kªßó?Ü©ilJÖo?ª¦›-ÜPš4FGL J1955.1+3321?î ̲±Õ@WŸß-øaÀ9ë!Ð4`ZÀ;U]"̃@6¬'=@o ×{|x?ȉº¾ØBw?ÔE,¥$'1@
yyh¡ª@	S§t£•ò¿æ±Q±£{›¿æxlâÿi¿â!?èÅQ¿å§ŸVqý¿è°ù'7}E¿ïÿýFKêOTHERsppSNR G069.0+02.7?ëlHÏKE+?¶'ÕXÿ‹?Mé{–~?v¼½,;?ÀLÓ£x…?´²Ï+"cF?ÝԟK¥µ?Îò'u¶i?¥À&kl¬í?°DÉ_¸?ßs[æíJ¯?Í¡¼‰ƒy?á¸Ë$wâ€?±à@΢¯Ê?¶5!Ö÷>"?ÌÖs0œ.?×!ARk]?°=|
å›?Ü	O2ÏÊÀ?³so\&n?hF€ö·ì?‹!´ßáµ9?á2dà?³Tóf
Q·4FGL J1958.5+3512¿ã֬͆@J蹒]eÀ9ÀmzVÞ3À;"ëü<üá@ p8Zdz~@9{Kй?¼vY£Š^?smóÔ#?¿¹¶š†T@2õ«hN?ï<ÌQ#ß¿Ýüê6jY¿ãí÷¿¿ž¿Ú¿
|?k¦¿å"}¾Ùû¿Öh,#Ê_ŠOTHERhmbCyg X-1?âæ6Éb<?ÀNÛCs?xâ5Ċ§?o‹í;8œ?ÙÐ	˜èÍ]?À>
ûz0Ò?ã›'^r?Ƶ:V³)[?}§ˆ†z?Œʖ­?ØU¡W)4?Ɖ¡wÆ.?âò<~c\?³/Ê.lìÔ? ‹^´¥¦?ƒ"¸84ˆä?Ø

ƒ"?²=_ë&i‰?å%/r¹`?¦ä~Ì\
?•8ŽÚC_?zIÜqýM?Ôbüé?¦UjõO€£4FGL J2002.3+3246?êr§ú|Õ¶?ñL] l‡À9u_€™"À:Ò;ߪ#@
+YuO@A\Á¡ö_?Â(ü8V2¿…®Ô5Ä)ˆ?Ãjt "?ði!#¼Ñ?é9Ÿ=Èb…¿ÞD­à#¿èær@U¿ê‹¼[f¿áª‰ O«º¿ß<À»ŸnOTHERsppSNR G069.7+01.0?Õ#åQÁ©?ÆÜõ`·@?"ο@Ì?–ïÕ´¢h?äϜ{]Ë?ÇHÎ…T9?řTkÎ?Äa­Þxª<?"ŸcÄNüÙ?Ì¢Xìc_?éô¿L¤¦?Ä¢KO_¸]?Ì©äë¬ý®?¨˜úÂiâ?²s½ìPyÐ?"º£ŠÎ?懊±Z?©žì™@"?½ Qôu@?£Ô_‰{¥?¡÷¥÷fÄF?1'ð:û"?ë>ñ–K?§Úà…=(4FGL J2004.1+2517?眾RÇ´EÀ	ÓAü#ÒmÀ:}–FþÂÀ;0ñ9" @–—G"ÎÜ@ °«.?Ô5Ä<ÛR¢?à¯/˜sÿ¬@	)5ƒo‹©?ÿê5mË	©?ïÈ8éU™?îM]®±Ú¿á‡ÜmSÀq¿è¿ø¨ó©°¿ïÿáa¯G?îRý"ªúÀOTHERunkB2 2002+25?Ìi¹ê©?¿÷áè
C?»Ïç©2í?¶Ñ¡1
Â?åk"43£?è7è&hú?Ëd	äځ?Æ#?½`¸?°"ý\¬b?³öÄÕo?S?ç[Ûû3Ô?ÆÛ¬­ö… ?ÑtÒ1¦?¬Æ»ãƒ'Ý?Æoxehˆ?¤uuyŒA¥?á©ÒZZ?¯zƒCSV?ËÑ8'ê3?­ÄÄÐ&«:?Ç#|æC?´?²ô힇`?ãBÚ8Ju†?¶ß×»‡&4FGL J2004.3+3339?ƒŒE¤¹ƒ?ó#5#Î;bÀ82(1wqQÀ:'µÜÆ?@¨=ý;ª{@v½+o"?¬ Jžðת?{Èù-©@"ßGù"Õ@&†pG?í%^>#Ò¿ÔM€flÆ¿Þ®<Sme^¿ä?'Q¦»Á¿ê;Á!Gù¿ä«¢æIu•OTHERunk3FGL J2004.4+3338B2 2002+33?™ì¨@RD4?‹ÊÞQá(£?ϱâ'VŽ'?ÃMó¨ðØ¢?çD"gÊ;?ÃPoŠ¯
?››¡võw?4bÎ?ÐìÇèÆ?Äf{‡½¸=?ç&{,Sñ?Äxf»U?¿1|·7?¤Óá6•{?ÈI=é¼?¬'CäGf?損n®T?°Íˆnþ>¦?¡~ça(?"Ø9
(ùö?Ɠ÷`³Qt?£(	§!
=?éI>Ôµ?¥•è"ÜÓË4FGL J2013.5+3613?š¢Iå}ýð?ðDq´xB1À9D5®7¶PÀ:ØÇNފd@È´p_Ž†@êC5öI?Ą‰bÙ?×Ò( °y°@zÒÁÙSÄ?øÅPt6³›¿çF3k¿Ø·Œž´`š¿á3€?ÖY¾¿çòøp¶L¿ì¯ú..ç¿ÚgzÍüwµOTHERspp3FGL J2014.4+3606SNR G073.9+00.9?{Iºú¬Ê˜?tÕuŸ–­?˜¥¦õܺ?—ÔPÁuÿ?ï?R\‰†?™ØsµúI?²ì@OB…‡?´ñ/'<š?µ‹7¥`ø?µŒ—
}*?êñc0?½ð ÿ+7?¹¬Ù²×?"´'uL$W?źvî¬}?¡ä¡ª9?ç[Ç!…:?¥¢ö¢{Pe?«I8®#Ã?—ÃDcw•?´(Ü>~ªè?£‹sÓÆ`.?ëÊßä¥Hg?¬é¨×£+ö4FGL J2016.2+3712?í+Yy–?ñÝݖH¬AÀ9+RFòÀ:Syú—á@"5g+Þ*B@—|ˆç›?äßzÿ¥' ¿©ƒ—àÃ
?ô« b
·?ýRAüNŋ¿ÝGµ¡7?ï-.Â
Q¿ë€#¦Î5ƒ¿ãÛù%k¼¿ãKêN½Ó5¿ÜsZÀ•ÝOTHERsnrVER J2016+372?vÙà׍ì«?ƒ¼9èKÈD?`×+
ûç%?‡ewSi?ïÁuEè??aÔ&v]?¶í]˜)?¼tÝjWÝc?¡r.Æî?°¯¨±è/@?ì1u0­?À؈]‡€?ÁT2®žt?¡v¨îÈ1?³Ä×mŸ?œi"6¥À?é2Xf·?¥õG&ÿÃ/?š'{çÏÿA?‹¨ãÙ5Ï?d»¨c^›¨?lB;àÉQ?ï¸x^!j?^Þëƒ4FGL J2016.3+4953¿ç.mÈý­@ ;EkD¹À:²€	¥›0À<`
šó5í@!èÀA¤?ø^h5sT?Îë``½Û?ÊO'åJr?üôÙáˆE´@XÛ¾­$f?ïðKAœØh?ïÿQ"W6?δ°¨©Ø¿Þ'Í»à¿È%6Æ:·a¿áБb"sOTHERunkNVSS J201619+495324?ä&ýDr(?Æè:?‹+É;_†2?Šdÿc;B?Öف»œ€?Åô!ë|µC?ã]1ÌhN?Í/÷y§˜í?{¿¡†É?'åÕÖ£¦?وGN´@?Í	Ò³…G?è–[íöXY?©Z:A•e¨?Ž›N¤¡&?y"ûðñ?˼Û]܍ª?¨'m'$†?ë'Õ©îE0?¥i>^ëU¥?ƒÀ×Ru×u?|ƒ2?Àx›ãÊ?¥$ÿ+8õ{4FGL J2021.0+4031e¿î"‡!®Ó@'âûã:ÍÀ6ûî'):ŒÀ9ºG²F8É@!ë$ ?ýþ«×‰¿1?¦ÙÞÃð/?¯BþñüÌ@Dnœ•Í\?ö}X@?ëIÒF‰QM¿êPãèrDÁ¿åŸ£i&4G¿×Mn]UƆ¿ÜºQ,k¿ßŠoŊ¹,OTHERSNR3FGL J2021.0+4031egamma Cygni?¡(…ÕøO?¯š™w¸?÷?tCg]c?…!¤1'y?îŧUÑÁ?±ÌÚ†\#?¡8¥ÿŒ?²Î®A'?ÐlNc*ÿO?Îå1ဓ?æ¶Nnq¿?΂Pýª?ÀÅþ?¦åòcÄüH?®Îܹbô_?•ü5a·œê?éá¡Dƺ?©MÈxÑp?høV L?\v_,`#?¦o
>ùš?ššíœdŠ=?î€ՑI×?›5V³u­â4FGL J2024.0+3202¿éÚ|λBÀ	,ºËCÀ9Þ Ž€`ãÀ;GµöâJ@ {¼ý@Á…pí©?ÈÚþ=Þ?¹E\U–_}?ö8N%'ö@"I­/?ïåÑ0é­?ʄ‰§‰r¿ä™þ³ú™¿è'9
gǏ¿Ì†£V‹}¿ïÿ¶ßO±COTHERunkMG2 J202410+3203?ै8W–?Äñ$Ÿ^ö?}^*ÄÁ?CuQ?Þ@~L=Î?ÄÞ{ ý>¥?ÔÞþ<rè?Äpá›+ÛK?uõ{‡O?ŠMQ<¨—?åd•êïî?Ä9tU¼õÔ?ãd_¶:÷Q?³wÕ8æ
?¡ºI…'Â?Ž;«Åµ²ë?Öÿ÷bæ,f?²ÓUåe?Ú[0åÎ9?³Š Žž`ò?‡ÌÒ+Mbw?€3gþ¼?âs4DkÇZ?³ª‰+@â4FGL J2026.5+3718c?å¿\+"¿àЧLàƒcÀ9½Í!†b…À:ßöX·Q;@ÔÉEƒÃ@¥
ÙwÕú?Õvzۓd ?èfÃî×¹@
me¼{a?õ°r‹ã£~¿äsþÔV"¿èªý¤Ûìû¿Ü`wIJ¡þ¿îø‡›jT2¿¾_~8j*¿Û•Ü
Wq×OTHERunkNVSS J202726+372249,?Ç:¢¹p:?ÃA|¹?´¾'ÉVåT?µ'ú¸_h?癆øyÆ?Æ;œ·ÚS?·üÔòe½?ºDñ<A£î?«÷¸ÒŽã‰?²¶Õp)¶?ë_äØ8Å?¼õ¶¦©C:?Èßdm3ä?¦"næ¾·?Å>&S'±ö?¦ÎXGrQ?äx´RF‰?®
"àܺ?È×e'a?Œðb-º?²]»Ê]VR?ª<,>Ï?ìÆˈB-?«í‹þ14FGL J2027.0+3343¿Ü´=-"jÀ8''
À:u¹Èä
À;…-RH¢0@#±"™ªŒ?ýgQbÉ"ô?ÅcrÁ¯Z¿®—Azž¬©?ð'¹M"‰?ú'Ÿµ<O¿îy`^dL?ïÚ­`ûH¿ì%V¿ÝÀ>Æå,¿àQù\wпá6—Á¨+ƒOTHERunk1RXS J202658.5+334253?Á6`K¸µ\?¹Ûàù_4?Q9v
=?I¸XÖªaÒ?ë©Ë2'?¹îŒµô®?Ãl"²®î?×£y]u?"Ë›²) Ì?¯O´OœÎ?ꆢYÂ>?Ãʞ¨|ˆ?ØC¶kÖø¢?±±"Et?¢Ák*`2'?‡]ìc'€&?â²n€†?±3¿{,ÊZ?¹\ ueí?¦|–%B?¢×¿^|Œ?£uÐèðÄe?ë°¤Oûkz?±a7+§÷4FGL J2028.6+4110e¿ß<Âݤz7?öW¾VèDÀ4–š9ŸÀ8¼ C@ZgPœ$¹@wkcü(Û?…kŒ.æ·? ¹L^ʳ@¶Ã ¢@wu2)ô?ß&2dZ™¿Ê¼˜·œcù¿áÔ<iÌ¿á¹n¡q€¿âqPÚãæſޏ¹OTHERSFR3FGL J2028.6+4110eCygnus X?¢h*‰-ÿë?Â4¿¼Êi?€uRµ|¥?´e€w–?˜¢?Ä©Cîq?Ââ'üÎöù?Í¢†¾<t?ÜKº¹åR?րԑ-?ÚBüçޟ0?Ó½ù™a?ÊH©ëì00?¯…·È-.¢?¸>GJǯ?£RÖ-ä֞?æfÜšþ?²º™œz?}À'¢¸€?xjÊü0ì?¾¶âTk(?¼òÛUg'?ëí¢¸w?½­´1S@þ4FGL J2032.6+4053¿Ò¯E'Ü;*?äO\"UŒúÀ8ÉRÄÈòÀ9ûtä®jâ@R
b""Š@´œU5¼?Łø4È?ÔNžÃO @óíx:¤@¨×Ðâ¿Ô(v;©Ï¿çIüm¤HI¿êêgèF¥×¿è–Ñ"qïÜ¿ëÀ©s+pÇ¿ïÇ/¿`R¦OTHERHMB2FGL J2032.1+4049Cyg X-3?×A¡võuA?ˇßR³rÐ? ÏÁ
'ÃÀ?¦ÎñÕÆË?ãR33âÉ$?ÌG0"¿?×Ô7Àæ¼?ѵ»?7÷?»Ü ZOf¸?ÄkY.W?àš`®ŸË?ÑJ©""?Õpüò[E?²gC
yZq?Ãw^w›?§ƒ^ëö?àiž/4w?³ŠFÕE?¸›³¤ç€?žàºšÕÀ?ª&ü̦!?˜aïᜰW?ëJ/<Êx®?¥²¾!tÀ4FGL J2041.5+5554?µ,Žqr@ é$Jb#âÀ:Ù­äÀ</êp'@2=²hŸ@^´UªW?Ð?ÐDÑkB?ÌÔÜeÇ6?ýeuU²Ê?÷ …[Ÿ
¿Á³k¢Š?ïäÂAÉy¿çL`RP¿ÞCиò$¿á!Äuæ6*¿ïÿîÝÃÀ	OTHERunk1RXS J204129.4+555144?æ|ïÝ¥'Ó?¼Æöʅuo?™±Ý²‹Ûû?œ4ä{nž?ÑkiŒò›?»¾Ì*uÂé?Ö38bùN)?Æ|ÒMñ]?«nÖ!Ʉ?¬;±†
Û6?ã/vls<S?Æã–¶/'?è#©fÌÐ?¨"‡¢ ü?¡ú{rnÉù?Rø	˜C?Êò»‹1??¤¦8§µí?ã©èÄV­?¨Áå4ðPL?¸6Ž&Ã?¡ñ¤ÑÉñ?Óé+Êí¡Æ?¦PE¤	q4FGL J2043.1+4256c?âŒ&ª	?Ô[Ý¡[YîÀ9;αð¨À:i­°hé@¤S³Ü;@O¡»§
›?×¢‰G;ÿ?í~âÿ>9!@Xt »ÌÊ?ü»ÞDno¿æ›å¿ê¿ÖO© ø³…¿ë}Žc|¿îÛ-M@$³¿ïӘc8´|¿ïø~a.ïOTHERunk2FGL J2042.0+4252cNVSS J204232+425813!?¾N	ðåÃQ?Á0E¬,Ñ?šÕ¾Ó"'?¢Ð}Lf?ë_ËJ3?ÂïõRf?§5ïwž ?²T>Uíh?Ñk§¼]?ÌÖgþ;?åÙ9ªwg?ÍC>¹×L°?Ȑ¨ž3|.?©?©øu%?Çß6=(±?¥ [lÂT¶?ãäI)Ç?°@6A=t?mç G'¸b?^1ìŽ1Ö?ר'ó¼ï?¾Çntfâê?ä
ÏV¾ŽÐ?¾´˜*¦û4FGL J2045.2+5026e?æí#b
o@®…bªðÀ6ÿp·ù1À:wÖåTƒ@¢¡Åâø³@8¿E$Í?rj֍•Õ?Ì&ãÚ˜Á@*è"úô'…@dk@?á?Ä/ZöñŽx¿ÖËF…¿å‰·~±áº¿çÏ°!Etÿ¿ïGšþôgF¿ïܛ¬™PžOTHERSNR3FGL J2045.2+5026eHB 21?†Z«˜b?ƒut.O5?æ`´ÀO!?Ȋº1
`?ҋÁú|ž­?Çûl{rñ½?–Šçù~8?¬!~d½b
?ì2o¸H?Ã@[xÊÀç?¸Ì•Þ"¹7?Á¢í–T;?Äh¤枀?ªŽ4sò?á,>Ði?¶–f®ÝâÅ?ÓË{œî?²jÕTuªê?aš§Ù -?QÍ%ýl?è½d"ë?³ü™"3Ö?ÌÇÌIØ?³ìYyðu™4FGL J2051.0+3049e?ÑÞ­1HnÑÀ ìµ»8OÓÀ77Ú¼y˜rÀ:Õçd'ÇÅ@¡ÓÏËZ@ž¸Ø#B$?˜¾"ºêø?ÉpÐãõè@-f8Éu)x@ˆÇÕGj?ïÁ´ †å¿ÕL@ËLD¿âßhæsg¿åÛ¹™ê!q¿è*'ò"È¿ê†Iàô¡þOTHERSNR3FGL J2051.0+3040eCygnus Loop?°5@¥—ª?¬!—+'4B?Ñå'ç¼Àß?Éô¦L*Ù?åŽwn­Û?ÉHÄ\6ş?Ÿ3Xù83à?³V²÷;و?ëÁ$d*X?ÄÌÛp2í¬?º*xž =?ÁgN£ûÚ?ЙÛ=+fÐ?±}—·°À	?Ót/AÇqê?´|°&Šf£?Ûñõ
'E?´Ö‰<±ÁÜ?k¼¦&Í?`ÿv%ãÕ¨?è0TY'í"?µŽ˜Å¤®?ÎϾC[®»?µiáí.Ú/4FGL J2056.4+4351c¿ï÷€ññ¹/¿ïDË ¥<À8âô2}À:¦"%¼R@ºvQëÛ@ûB+»?Â)Zl] ?ÓÆ¢[Šk@!w~¼ž?ø-c­úN»?èáºÅc¿Òô&­é²·¿åá?(‰â¿ë	ë;LÝ¿êåB_ !¿ïÿÿ>¹úOTHERunk3FGL J2058.0+43471RXS J205549.4+435216$?¯ô3·«N?¤Y-G?¿8f‹ Ä?¸o§ÜˆðJ?ê²ëd!3?½yÐ;Ww6?¦"¦k+Ú~?£nçE0Þ`?ÁÃQ¡—ß?¾c¶—Þ%â?ê&á1Üa?¾îl  `\?¼V·Æšo™?^+¡ß*Z?Ï%á6?°}?¬þ±>€ÊJ?ä«°¹œÅí?®ë(dÍõ?ˆ$'6¼¸æ?qU¼'ɕ?ÌÇÿ|?®"Ó±ð8?蚽cF×?¯Þá{34FGL J2058.7+4454¿Üfž›GU¿âçF`6¡}À9t— Ÿ³À:þºoÒö²@«œÂ˜ìK@7á2µ^ò?ÐÔbãz
b?ÉH±õ…þ‡?û}E‹$‹Ñ@P	N][%?ì¡ÚƙØ?ÝjùÞ}Ï9¿æˆž¿É.2¿ç»Sþ"Õ½¿ïø*~XËs¿ï–ü0g¦ØOTHERsppSNR G085.9-00.6?Ú3ü¸Nóë?Ä[Äz™K?"–Y÷È0\?'"ª•ùö?âANÔD‡?ÄkŇaÅ?ÖDå9Q?ÈMuŠ.?"8õWú?œ5{í`ƒ?ä;̼ۍ?È´C‰†Í?ښ!\@¤—?²Ùç¸8Ù?µŒi²ÕS?™|®xÝ£?àbŸs
?²-ß|±Tâ?ړGäÊ('?²|˜B8?©F>t?"2•Ÿô?á$空«p?³Œm¶'6ô4FGL J2059.7+4837?ä2J9¬k{?ûF8Éu)xÀ:º}SèµÀ<T«@‹
‹@ÝÌÃèw£@‰à¤&?ÔÔ@ƒþ¨?îh—c^t*@¼8zšÐÑ@ªæ:²œ¿ê`ª?.>,¿ÞHšu%F¿È¢]b†²â¿Þ¼£¿ïý²6ci¿ïºýÂcOTHERunk1RXS J210008.1+484122?ÐÑý3€²?À(ÉB°?Μ[ÏÌ°?ÁGÖ²ƒäö?ßßÔúæ'?Ä*"o¦?³í€üã'?¼œúXKdz?Ö5V¯)a?Ϗϔ£®¡?âg¤¦ËÔk?ÐHmr™y?ßé¢ÏMÆY?°,}€9•¦?ËIžL=n1?«jØ9–?ÒqŽ
"'?©í»O•:1?Â5FfŠº´?¬-ïÝ	ïl?â;šè´†?ÀÑG\a?Òn&ûR›š?»S"×T4FGL J2123.9+5158?î"Â=?óhG7À9ó¼¾aÐÀ;
cûRV@¢ì1l½@¡¬Âk?ÖzРìÊ?á›Ό@@@Þ$
%'@5òzÜ?1¿í|ñýþ?•·©=ë6ß¿Üàû㐳—¿éѺ¨¿ïûR}ÔA¿ïqNŒU
yOTHERsppSNR G094.0+01.0?«wˆ/¦Ò?¢`îP©û?£!¬Ú?¡ß(ú´ã?íl¯mÔ±?«™óQùK?ÇóíZw‹?È:^Ÿ4I?µ–ðä%+?µT9C¬)?çP&§þÝx?É¿ZSLYo?Âg÷›ïaä?¡'æ½a<?Ç®"3=/<?¥U^ó
^?åz]4Û¸?©¦LÔn£?Â:Çÿ["~?§¼øšŽ«´?¨àdÌuÙ?–³GΐUÀ?éãG³hcƒ?­L`7ŒÄ¢4FGL J2129.9+1208¿ášSâÄõ'À;Q½aõ¾^À:1'"ªLÀ<5š5 Ë½@í§°³''@?"äMòÒ?È'amÙ!?Î!µz@OjCj¸Û@ï/1?¼§»rÈ¿âè
`+8é¿åo‹^¿¿ìò_c<æ:¿æoA×:å¿ïÿ»!(ĚOTHERglcNGC 7078?ïYí³ªm,?"nÙ¼˜0?nñ	üŠè?iÛÿü?ä(K!×?'ØÀ˜oa^?îéî@Cª?›ÅÇ?'©?k$XVRï-?x›™'Š)K?Ÿ]³-,ü?˜ß	·©?íó'0Ð¥?˜\"3h?ç2\·*?"}öĉšü?©£&^%?'ː2…v?îc)h¤?†ÊíÞ{<?x̵žÓë?c	îï?¦³×…£øR?…dñð	4FGL J2217.5+6346?ïæ`:ìÿ·@7hiÎÑÀ9Á²'ž«QÀ;ÆAÖd%D@!	ò«¨?ý顄I¦<?ʊ¾	w‡?Æ*"ÿ%À@I"¹`~@×èØñô$¿ï{ Ôvd?ïôx½«ò¿å/ù‰¿ÛõsŸ‰ó‰¿Ø§–ýˆ•¿ë?o¾ÁÇOTHERunk3FGL J2217.2+63461RXS J221728.9+634714?ï1¿‡¥ÜÎ?"•†Ñì?MŠ¥9Ú²ð?L"ÙIØðâ?˜Û¹áuµ?"M2Ü`?êӚ/òni?Ãà_(ì:z?s÷p|é?šeqHLð?ÄÛ¼Nýý?ÃfÀ{zý?ꂪ –ÕÅ?¥!Ö;¯›'?'µÚ#Eé?'÷û‡]@¹?þœ9<?£XÎ=h¾O?ë¼1VbÀÜ?œªŒê)¢y?ˆ›r
]Ôé?|U=OŠ@½?¿ž>…?­Š3~4FGL J2219.5+4653¿í°)Î?,À ÙXS~,VÀ;W«p_À<ˆé¦!gY@ Á"ý}™´@ÇÄ\»Â¹?ÄÀ¼ؑ|¿«å'²¶?èåRŸà¸@œw!ŸŒù?ïþ~ö€$~?»Ä‰1l‰–¿éXޛ¬C¿ßêÙþ
·y¿ìŽ°Ëæ?åÄ #!OTHERunk1RXS J221919.9+465137?ç½ñÚF)?Â	ˆL9@?xâ^nùyË?tÏ "`Ôì?Ð 'Ñ·Ç?Áùí²¡	æ?ÝÞç,—ôï?Êã`"›?p›[LšŽ?€ˆ¢«¨žä?àïU³Њ?Éû"(ü!Ï?éûòU{?¥4åܝ€?–êuH?†I¾BJ'"?ÅM¬	Ó1?¢Ÿ±ìG¦@?êڛœÒJ?¨×^¯iáÂ?-6CÌ­*?†E ¼¿-¢?êÄ=í3?©×$wbA4FGL J2241.9+5729?êY©KIñ¿ñÈ÷ŠæxoÀ:!´¢3œÀ;"¾â(@Ûé	ïB@ðæ[L?Ïfr»3rH?ËÙ©T!ÀD?øö
³¸)@¤[›(¿ïd~š9Ҋ?ïþÔò5<"¿èӐÁê¿çŒ>'Γ¿îò-Lie?Óª¿^UKOTHERunkNVSS J224154+572700?Ô^\ºlO`?Ã+)%Ã"?ªš¸ƒ0?¦Þ0­?ä/g÷A§Î?ÄiZ)MP?à:if?Í$°Ç`Xí?'—	OI-?¢½Ï±á?Þ¼˜Ì™õ?ÍœÃć?؎8–¦©4?°èÓúBZ¶?¹ð¥~íe?™òÍӂ¦>?àzÏÏ9?¯m<NS˜"?ç€Èjkî?«B€þå?¥åx7Óñz?"=ê)Yµ"?̃€IÉSå?©	7Â1ì4FGL J2254.9+5802?׎Gmx²¿ö…È̍íÀ9úùXF3À;œØ_¨D@çõ±óW¦@ål†;?Æ5Ÿôým?½ó"Uâá?÷rÉìG¼W@?7àÁ÷?ïÀ"¿óuƒ?ë§xª`¼¿åÄíz¹¿äM5<ø®Ó¿ê'`eŒ¿à_ô¯iåOTHERunk7C 2252+5740?¸•~<4p?¬HÍû•C?®f2×?ÁõG3¦Ø–?ëü‡7ÆD?ÁŨyP£?˧¶±Íh`?»fû•½ú?‡æÞÒWCÆ?Œž›7y±é?è¶vØCHÙ?»‹Ï3=è?ØV3'ãN?±ÿ:˜Ï?®¿ókvºä?:ŒSíê?áèçE"ª?±o·«Œ"ò?ܸGäwæ?¤Óúæ{n?µ
¾}Z?—¯Øºl@?Þµy–¨Å?¤É'ŒAÄq4FGL J2258.6+5847c¿×.¥4"—¿îSíPÑÀ:<§Û{¼9À;ŒV=#vþ@ E)ØÁw¯@j[{PÙ6?ÔxžaÕ]?Æ0C>Ä?ñ¾Â³nVö?ñev&wä?Ä8AåӃö?äÅhT}0¿æµAjÙh¿ÜýI׺f™¿ëqáÄ«–¿Å!]Þ,›"OTHERsfrSh 2-1520?®BaUSœú?¤*¯gñ?©Ùü¡µÐ?¨
ùéñEÐ?ì~: n?±@'Ïv»º?¹ÔꎥÜ?¶8,œÍw
? `V»{?¥è4mÃ?ë¿]F9XÇ?¸OpF«?Ôz!µãí?­ÐʔƒnÉ?³{³ÀÕɯ?—;½'Ê1¢?ãLw
TÓ?­2ÖÎäN?ĺM)§? yJìR?¾¤×Ëñ?©ës^$—r?ç(ÑÅ·s?¬§ÑÊ´ºŽ4FGL J2301.9+5855e¿çY§bœ¿ðy`>.9À8¥ÞC¯'À;jÄ$"õ@ "öøogí?ÿµè"¹7Å?¬AÒ³@´¦?«"͏@'2úÿ?@WÚœ&¿ÔEìþñb-?êÓÌ@
>¿ÞU…2à'¿átA ´@¿ã3>)[n¿ÜÔ¢¯OTHERSNR3FGL J2301.2+5853CTB 109?ÝDáA9?Á)D˺\?'"‹Øe9?Š¬µ#¬@?àîI0~¤9?Á6
-d—?ÇDÆ܀¢V?Á´r3è?¦á°[U
Ç?®E£?èÀ³C*†Ž?š["VÑó?ÚT›Zî?²¥ØÉLƒ%?©¬" ë¯?OeŜ6!?áDÕwCÎ?±¯S{ì?Ú¦òÉ'"?³«Ôï?ÉCLÅGà?¬7òt½~Â?ØÓk•É?°è…Ä"¤-4FGL J2315.9+5955c¿Òüáøƒ		¿èOQ‹N}À9V®ÃÍIÊÀ:öÕsd{«@b‡üŽ1@jî+¸ë?ÇΊ<."x?ÇõíÂæ™ý@˜ÿàöO}?øÀÛ­:`N?ïÿÝe¡D‰¿æØO·Î8¿ä»P£‡¿é2*õw¿êìóžGÔ*¿ÞŸ‡ÜôOTHERunk1RXS J231543.9+595510)?˟ÎF}ö?Æ~FŠÖ;F?—µ#Éyi?"gƒâ?èZdUB6²?ÆÃé[L?¶ÃQv'oò?±úÎ"ÓÝ?¥ÒÝëǁí?§È…
Π\?ëÊgòq9â?³GÜ—Íš?Î"×ÓF?ªtô<úŸ?¸v¨J¾ò?—2d'Ãb?åh¸õ֜?ªæ¼—ü*?«çIøغ!?ŠûÒ¦ðž?Á³¹øèZ? O±¾êx?éԜâqzG? Ösؖäó4FGL J2323.4+5849?Ë>ªŽùyÀéÛÑLŽÀ7'BÁE°
À:úïY­@ۅä°ï!?ýîy	×W?šKc™å?²³	¾U÷¿@5¿jäz?ø:Șµ˜ÿ?êVð§h[?ІÁOÁs¿Ø€Jþ€ùæ¿ÞýD
öä¿ãÒRþT¯/¿Û‰°b³ÔXOTHERsnr3FGL J2323.4+5849Cas A?Æ""ì¾F?¶¨Ž.µ{?¥¯Ä'èŽ?ž›u)|jF?éb½K¡æ?¹TELlÅm?¹Jç†w1Á?ÌGwîÙ?ݽ(?L?ӗ0æÞ,?ÛðEö#(D?Ïà–,-?Ò&…AlN?±W1ъ"E?½‰86èM§?¢ñ¼ÖÎ3??ã;–Xlô¥?±Òy»¨h‰?°ÙHÿ¸	?—¾lCÙý?á$Û|¢¨Ü?¾‡ :
u—?ْR´zÀG?½|Ô¸»'4FGL J2326.5+6122?ï£	F¤f?Ì9Ê&)_À:â¢÷ç-À;Q·ê½xœ@›, šTU@3«ÉGO?Ɍ'sZj°?¤~=šZ?à91yõd?ÿÄ¡ÿ?í¾áÝU03¿áÚñR¾¿ê7A_ƺ¿ßÍbßHOz¿êÅV¶Jª¿Ù±Þ´Ö·OTHERsppSNR G113.0+00.2?ÌÁjÕ¬õì?¾Îá=•¦?ŽÌ"t½²?…
­ë«?èWF
ïŽ?¿ÓTwÉM"?ȏo‰Ãœ?Á4yó>?"¤ãµfðy?j'bbòÿ?鉐¯GóV?Á
e®,s?Ôr¨"dÔ?­+;2ìr?«î`Œ¦6?‰–:n"úã?ä>૆3?¬ÑÃk?É?ן8•C?¯Õuµ@®?¡LÃârW?‹ô\'Þ/S?ã°µBŽ9?¯Ëk¯{×4FGL J2333.1-5527¿ëAÿÛ©ÀM)f@¦¹=À:I-(W7À<Žï¼»Ý'@í¬АÒ?ý»í·(Ú?Âz‹÷Åsè?Ô°"‡áá1@ÄÖÓõ¶?ø9‹¼â¿ÒÜ"'Z¿É§<µ¿Ü\2/ýô¿ãv=öÔ¿ë‡'aBæ¿ïý|Í°ø[OTHERbin3FGL J2333.0-55251FGL J2333.0-5535?Ô³ÇOU/¶?ÀËÐ(•^l?Ú÷Ê/øȺ?Ç3¹EÞ?ÐTn€²?ÁP?K¬¾—?ß©ëۈ6ý?Фjéü¬?×Dc#
?Ï·"¥9v?Â#a(ÉKñ?¼Ï|ü˜àz?ÇÖト?±(Ö˜?äHIƒa 
?´攊Ñ6?ÇÕºû×?§s^¿	Dz?âOè6Ñü?°‡žäOk?ÅŸÂÄβ?«³Áoxei?ÐÓ_°ù v?¬1‹"šÂ%4FGL J2357.8+6231¿ëÄ;¿ÚÝ?Ó8ªŠÀ9IëoOCÀ;0Úb·…=@qC~Yø@èÞæªÄd?Â1›X‹‡?ƾ	e"i1@QBè²Ü?÷a,Ór®H?ïÐøuÈ9¿ât1€*²±¿éÚ]C§õ}¿ç…öº «¿ïÿ4=ŸGÙ¿ïåﳁ¢OTHERsppSNR G116.9+00.2?æӜ6ԁv?Ä+[!v?¶Ë?t®M´?µž­ýþ€!?ÉKïjVÓM?¿´€Åw£Ë?¯÷ÑÿLmð?³¡ˆ­ ?À%fdØ­û?¿kÇý–;?é÷)FÕ
¡?©ÞG1f?Øîÿa	J"?±EëÅØ3‰?¾nvpš?Ÿ}pÂɅ?ßuzZ²‡?°!ËtxÐ?­NÔ_ùn?ŒÝž©¯:ð?ظ®'ð@?³§¡9×R?áÏb¶ðÿ?³¤´	 4FGL J0000.3-7355?ïåFýP´ÀE]a€M˜9À;%¦Ñ€ìÀ<ʞœ7ً@ÇÍz3£@f»üÊ?Çõ€ #v}¿®0C(É£?Û
ma'Pþ@ #¾ööA¿ïîa«ì?ìª'á›eø¿ãJ<߯R"¿àÖöâv¿ãڏÎ>¼Ô¿ïûSÞNjUNASNone?ïê8:š?cþD¹ñï½?>u"DÓ¹?;HFœG¨"?bÝF9?bFÎ÷»›?ﺑagA?ƒìÑ+ç»?)d™yÔ??A$(5?€öU¾ß¨?'•	i"µâ?î5Øù.Z­??ýç,W?y]ŸÇ¸?p,Lt+ñz?©v¼Šátá?Œ²ØsX?ï³caj²?mTú¯È‹Ð?XÜMÒ3?LG(ƒ÷«‰?€¦;™5?l×F¹0ŽN4FGL J0000.5+0743?ېÇÞ{uíÀJƒÅ?9ѳÀ:πhp+âÀ<t3⅛¶@»?ö;\?ýl½³TUÃ?Ø·G?Ëç?Þå¥vF®:@JFsBî@ÿ_Y¬Å?ï¦'ÊÖ(¿­O·½	úï¿à)HÎ¥êá¿æ™¸:lã¿ïÿãzŽ;˜?Ù­ µTUNASNone?î¨<*`á? ôÄZÁÍ?hnE}z?dêm:ã?£ûv{'M?ŸK"pd-?î·LW™^H?£"£Í̖'?qù¢‰-9š?'F¿š†M?¢L5Dt\? a@ÝÊ4?ëϘE¯?¢b"<~à?¦‰ÿHz?¦?""VœTH×?¶B™•cH?›K'5Z_?îF0à$­þ?']p™?nR'¼¯?evGŸ¯æ?©·ÏŒ‰W?Í"5#–Ô4FGL J0003.3+2511¿êÞ¨GîgbÀB4«ùiäÀ:¸üþÿÞÀ<|ÆÖƬ@šº²˜îú@v€$}Ê?Ð>.ϏÐ?Ԕ6ê'@\¯-•?ïÓێ¨ò?ïƹT繿à£h_Ýƒ¿à¿½‹ç)¿çk½¾<¿ïö({ILz¿ïÉÏ÷úxUNASNone?í¢)=Ã_Ü?«¡Ñ{úÈ¥?ƒÛ>auÃ?†®"ÒY~j?°sV
Òd?©æCà"f?ãF´Šxô–?Ð-™žhÙÞ?ÉûàÙU˜?Êï˜-N4i?ÈéM¿BØ?Áø	¨t?èý+ÞI?¨wUâ7¥?´xHì?šSI±ºÓ?Á˕Ԃ˜Ê?¡D¬¼Ç?ÔkÏ •Ñ£?®ÓßÕÕ?ÑVbLÁÙ?µ­lN¶Å?Ú=ÎÀl'?³æ£RæÞ4FGL J0003.6+3059¿ßêf-4À>Å¡fµNÀ:ô™aeu¦À<ê)\ðœ@fçŒí?ýK˕•(?Ìu9èÙó§?èŸüàõ–@é™Á݅'?ý})vpö¿ê!—à¿ßAJ¸Šöi¿¨€Ua¬{¿èïÎY"ǿ隢ãÅ6Ö¿ðUNASNone3FGL J0003.4+3100?ÛN< °Ò!?Å´z0ë*f?Ü«JÙà=?Ç
ýH™-¬?Àñ
Ýàƒ?´ðŸý}"?×pÊí`Å?Ëä.X*(?Ú÷"drށ?Î5	ìL?Ë/c1?u?¿÷8ýÒsÐ?ÒùqÚfÅ?²ïÉß~<?ᩅ݀7Å?µKµ!r¶´?ÃgTJSd?¤SG‰x$?Øù§ &Am?´' Q@ÈÕ?ÖLBì¼wb?¶àïm?кsG1?°°‡Fژ¶4FGL J0004.0+5715¿î°OÎ}Àj<´¼5À:
ö¯õ%±À;øãȑԩ@²á±
y@éÜÂä¿?Ée¶h1m?˽®·8@œC²Ý7~@Äó  ¿»ž#þ8?ï3À¶‰?¿æm4§§y¿â½˜çÂòX¿êÄò]€
׿ïý."hqUNASNone3FGL J0003.5+5721?ؼ/QbOé?¿â¡ËÕD?»œBd¶?±CŽhf3?à?"Ö†‹u?ÁFøG«Þ?Úk¢03P?Ç)ýÊg³?'VÝPɈì?˜KÙO=–Ò?â7wý`y?Çã8­7?á&Ýì½?®÷uÅ$8?ºÒ»Þÿ'"?žµi"Åj¡?Öý–Êf¡6?ª¹'MWñ?çRÅ]º?¤Òtž]g?µ,-ª?«V?˜"üӁÐ?ÈÓ´iAå? ¬ø¼¯sH4FGL J0004.4-4001¿åU:$q¬ôÀRvñ€
À:¤ˀœsÀ<¤@è'œ&@M®$ëò­@Ò=ÕM¤Ï?Á(òg'Ñ?´Q
u#î?ñ
	n=Ë@\nóӡӿ؍«dGRO¿â
M++ýµ¿ßdb–£¿ÞÇCuö|¿éw±b
;R¿¨ˆ¤B®ÀUNASNone?ïÓ½»ãNÁ?q&ãÐ]ñ1?IÎﶬ?FºÛo…å?rçD-ÁÞé?o‹yUçú6?ïÀ½uRN
?'¬ælE?0bN·@?GÐÏ}¨Ý+?~ŸO1í‡F?gÊ¥T'¯?ï2UDÔÃ?~Û ¨Ú[N?h>Ìøg÷n?f/s¨3
?–­}ÆpèÇ?z°áˆœ–G?ﲂöm‡å?iȸ'¢hx?A:\lq©?1½Ôãž(Û?'KœÖì?iTžq «4FGL J0005.6+6746c?æí>¹=È@ åæyF=À9»g
USÀ;8Ś©d@«sP¯šã@Üï$©Á?ÎÿöZdÐd?Ï}Æ_@ð?Û¸"@ó…PalW¿ãŸ£i&4G?îÏ`%Æ¿ç
.Ýc¿èéRáP¿ëžÙßÚƋ¿ïÿ/?ޒGUNASNone8?Ôה÷¶¹4?Á"²Ñ%|?ÃÅ2 •°d?¸Ž½Fóöê?à¢èÛÿ7N?ÃƬæÐ?Ñ©ýþóuþ?Ãå´"$A?ÂGã݋Y?¾!*€Ú­ð?â™>Žâ+?Å· Öæ7‡?ÑKéuð§?­bjÔvRS?ÁØÕó9`Õ?¡|]VÚ?âãÕȧ/x?®ßã£¼?ւ\€??©íb€<3×?Àûiœ=Ú°?¥´óQ\i?àÖêãI4?­8?Ä4FGL J0006.6+4618¿ÏñVf`~'À/½KÏknÀ;;·"¤%À<"g©\…<@ u™Y,í?ù,?£ƒþ?ÝQcŸâˆ÷?âi9Ÿ³äô@$ë7ò@?ù\ͶW¿ˆf_Ÿ;³Ï¿ïùš@¬ó?ímÿ"Z¿ÑÈýú1¿â%¢@Ýî¿ïÿñhUNASNone3FGL J0006.6+4618?îÖÑDêW ?œ½ìâts²?€í'oۈH?{ÕÏ֝Ø?œ¯*ÇGÑ?šU1áâð?î_æíÀ»õ?«˜5InQ¨?w#Rk®ÈÛ?Œ$ë·xÇ?§&Ö~g§?©}š"PÃ?ì¸ùlÜ-®?žé•‡NJî?˜k•€B?€@E—?:-?¶7N~92?›Ç´J	aë?êS?"ü?©ú(Ú.Bâ?qîþ\'¯Ž?m¬±àcÌú?Äû9˜ޓ?ª<ˆö_á4FGL J0008.4+6926?ï#¿ÝG°@Šü‹y£À:S\лnÖÀ;¾=‰ÎJ{@ Á<JÞö@ïþøþ"?Ê	¢Ö"0§?¸—=í§?ñi!—)|Ñ@¤5ÂÆ¿íÓbÙð!?ïþÚ0bž[¿å@£(Ž"ƒ¿åôûTŸ"…¿ÚW3£E"à¿ïÍbUNASNone?æeâ	AË9?Á;g¡ä­?"ßo±ÄaX?£ÄP©ùÇ[?ÑöDò`#y?À¸Y)Ñm?ã9ÒÑ0#!?Ë°K/þ£q?z®ìP†?ˆc'¬_Þ?Ù!ž¬_IY?Ë_Ӏè0?â.IrRË?°¦öÎô°?¨#
9‡ís?*ä4o_?؟t*Ò¼?¯D=R}±3?è©

Ž¸?¦eyÚ­?'ðQĝ-I?ƒ¾֔¾e?Ë͝1ãu?¦gõß
€Ú4FGL J0008.9+2509¿â^…›N¿EÀB\¿]xÀ:§e
EÔ À<K>I窟@îÒ09@" 5•
?ÏÎç"3*û?Èntý­ë5?ôÔb³S@â±³kÒ·?ïBO/èû׿Þf7l}ל¿êDP\8åû¿í}‡Ÿœ¿ïþž5àŒ¿ï€ú)&jUNASNone?ïjŽ‡?¤J:k÷?cè]Q;ç?b͸Êöž?@,SD°?¤$ª›à"?í ¨0³D?¯0±‰±?'Ñp;v?"!;¢/?° Ñ¾~x?ª']:½Ö?í
Ýw‡Ð=?˜ü«ÐQ¶?'vi?€Ë\vhž?³Iö¾§7ì?•9ÕU‡Žï?í¨"¾çëŒ?à+.CŒ?;Ð6i–?{Òp~A`:?­Xì)fƒ?%T7Í$-4FGL J0009.1-5012?ßýÓÎQdÕÀPbç-¡"ûÀ:kõ²Ÿ$À<'ò®2®@ K¤ï
?@éÇ´_?ºÃˆ€l¡ê¿¿:_nÇÖ?҂ú;h@	S6Þ¹^?ïÿlýY\"¿×ö%ö4¿è>O ¿äöTðóÿêY*ÿ1£¿ïÿ"¯ý‰-UNASNone?ïêü
ºê?n›
»}(?A´e¿;«?Iû©–\ÿ?`–ÛÕG¿?iE"#´Ø"?ïËØg=?ðaSÏ?-o©<ð¹?HÏB?y+ógyÇ?€J{)fg?îûß3¸q?†ü¬æíÚÍ?vÔÔdj?ssóõöw?šÎäoÔÑ?'Çdl+%³?ïÐÆ¥8?^¬™ô$¬À?U$Gæ.?Fiiñ	?rS›¢ŒŽ¿?ZûÏá4FGL J0009.2+6847?îÕðЕ·À@ðù£v'À9»œ`ô6žÀ;f?Èc@ïÓ^y@Zh+b"?É$•vjN?àÕJœ@iž»'?þ,­.vá¿Ý.Íb¿ß%"?]ä¿æ¬\꼡ܿì¥×€D¿ïÿ'`4P¿ïöU\Rç.UNASNone3FGL J0008.5+6853?ÊïF‰Ÿl?¼Ýn;?Óê¾·¦é?ÃE"¡¹?ޞFòƒ‰`?Åò€|ûQ?¬åŒ'}'x?´~"ɖoË?⛗@+LZ?ÌŽ·,Æå?×,íY´ü?ÉØ `í	?ʊ$j'ê?§î`¼¾úi?Ó'nQ¹Â?±§'´¦?ߓxÿLJ?²ªÛ1D¢~?šø±æ)±?€ñ^'Mxî?ã¨Å
.m?¸=iٟ}?Ø,zÇ@?·¸ùˆ{a4FGL J0009.2+1745¿à#Þßý_ÀEû‰a=1ºÀ:ÊZõ1À<ulC9@õ'ßÃ@fàÄÑUÉ?Ӊ7³Ët?Öüàü.º(@±FC±/¸@uQÄ?æPËßçܞ¿æ~ُRá€PB¿×¿ëb¤À>I¿ïý¯ùWoS¿ì0>·çUNASNone?íACìÉùÍ?«æ?®*m?zG¾:'?xHº…û¾z?´Qd¹^=î?«gþÖ#Þ?ì¹0¨~tÌ?²í}šüÃ?m¿e3š?"›Îr£Ô?¶ˆÂÏi"-?°¥
l?'?êÛ	ük,?¦ð4^?¨ð¸Q'AÅ?'DÔ¤+?¼¯[o‰¸? ŽT'ãZ?êþ¨ØD? ˜îu…n?"¡µ»¤ŸL?ƒ¢ƒ?Á'(ù*[õ?Ÿ2«0Ð¥4FGL J0009.7-1418¿Ü
ò®~ÀRz^³¾#À:y?Æ¿l'À<Žè´‰ßè@"êžnëp@{èäZˆ?¾ñ[¢h?¾}¹"6?ù[åô»ÿ@1är…Ùs?ïþð çkµ¿Õ÷Å^nuT¿éç`+¹Â.¿énlŒñ¿ÖÄ¿ðUNASNone3FGL J0010.5-1425?ïU Š¦}9?–ii4<?b؈3v?ffÊYG('?"
tÖRr?•-~Ȧø?ï?ÕåM¦Ÿ?šHšÊы?_Íp_UÅ?ru§¦g‰b?–lUU6Ë?—©¹*&?í<qÌïÛ?—Rµ§îâ<?ŠŸG†ˆß?{ö•(µ?²ÈöG°?"b¿º‰ðë?ïTÍ Š5?9»lÄSž?sê\¯ŸÐ?h9ƒè#/L?˜úäôÂÑT?~§ð*áUŒ4FGL J0010.2-2431¿æl½Óa«ÀTô±î$5À;}íÎ¥!À<àINþjÕ@CÇDø'ˆ?þf ³iNx?×kWÅ®K?Å2äƒÍªm?텯¢šÜ@€­ê´iT?ïÌGkÏ[ó¿ç`.ßœ/¿åÎ=_Üßj¿¿ô/7w)¿è
˜à66¿ïÿ'¢."'UNASNone?ïÊh¹¤xa?rޏdô¦?ENÄÚªn?@*€¸$þ?x!ʒsÚ\?q÷8Ç>ÐW?ïqė[t–?'¾öò¹´›?M™ö÷»Ö?]¡ÀžI?Ú¤œÙ¯V?â'
Ut?î'†ȲT?ë({Å4?u°`léÓ?f /¨*ææ?ªÑ'× V?‹ûÎûHœW?îžñŠN4?-µ:P»?W¤ÃÁñ_R?QˆY(¼d$?¥SÈK'Ä?ÏLB"b4FGL J0017.1-4605?ïô$|áýáÀQw_™Ã‹À:×íø–3À<©å
5r©@¼‰:Ѹ@*╶¶?Ã&LšãEµ?")ÛÔÁR?νÚÁ'ï?þ¿VGµK?ïäE#öN¿ê˜Ô½‡	Ÿ¿è–­Í-E¿ç]W>UP?¿ïþ‹ Z›¿çºñ£EêÆUNASNone?ïôˆ=^о?Rfüˆ›RD?F§QY|ý?G'Ÿ1±?G7¹+¼…ì?G=²è'8²?ï-,+?µ9?šE2Q}Ç?dp[6+ç?v
kvÊí¾?—Ìo8"^?—n&^ë~?î	¿,Ê?ºâžàé?…ô½šÕ+?}Îø£³™Î?ª†ÝÙ.?‹×
7–ó?ïø
†?ƒžù•î?†L–è4G¬?wåI¡ù¼?'z²éµ
V?zyÜý›¾4FGL J0022.0-5921¿ÚAê‹y›LÀL°Èÿ¸²dÀ:sÕzñ7æÀ<XCëè@Ðu¡æv@…qŽ¸•?ÀŽzV³@	? !ÆyK›?áuÒ"4Ö@Wj^B«v?ïý)‹ê"n¿éb"¿H¿åVŒ¿ª¿åF^ˆ¦¿åDmþ5O˜¿ïýÒÞߞâUNASNone?ï†5·>Š÷?›ürç¼Xš?Z¤n-âÚÓ?l^\Ió?‹j ç#?˜«üÃÿ¿þ?ïkTÍ6z?'-ô:ò?L4$OHï?Y[Ú¸\²°?'³Åpvw?'[öVw[?î4¼e<?'1ÛþKs?wþ~ü…w?f"øɶ!?©´iîü®??›±×?îmõÃk5?ˆ×_
P?ur¢¡¦}
?aŒŽ·``?¦rZ_"}?ˆ˜<Zúr4FGL J0023.6-4209?ÄÐÈq•»áÀR{½øôsÀ;kÿñÀ<ޟ›;ZI@â#P<@Ž­\Äüõ?ŕá"!¿ž¾¤k?Ú*Ÿü4C@ü‡ìóß?ìÁ?ûÅ¿êsÕº²¿ÌüòCÿ´+¿ã±L]üŠ€¿ïÿ Âg%?ïý<Á§TÃUNASNone?ïԏÏ¥?p2Õ	ÑÁ/?MßÐRcÌj?IÁӊŽC?qüy
àù?m¬`ŒY?Nçç¢?¸'µb?DšUÿÐc'?Y¼)èÐÚ?‰Ó†æ	b?Œi-ø"1?î.ES?•+÷DãE£?†n'£7)?ƒD"Aø7?©¡vRࠍ?'öH±Ÿl2?ïo¨5ˆÚ?~íò¿æ?GÙÙ·Sö'?BüVár?'L**‹?}÷ªšé©e4FGL J0024.1+2402¿ÓOÍO¦ÀC4äd™ÍÀ:ÅÔɐ¥À<œ!ªt³0@Þ|§E~º@$™Ì¢Û?ÁN«^½û¿q)%ñ£"?°Ù•³%"@V½ÝñL¿ëKYš¦	?çÐP~¿ê¯ ê[S¿Á"Š‹ßœ³¿ßJâ«¿ðUNASNone?ïó7M›=Á?T'ï•b'–?&bûQ©š?!k
û?VÅ_b()?S;ŸŸ}‡%?ïÄË£›Š6?…J±[o"?#Ïeðù`4?>2Ú³8ÕÉ?|û³³š?"ùCÚ¿Õê?î⊆•ò?†à pÊ}?jw?"%°?a¬þ»Á'? /æӝn'?…šõ÷žýÚ?ïÈx˜þ'?bñÌF
7?IÛÌ}ú?>ñ"QçˆB?x‹@™&Õ?a¡C{¬4ò4FGL J0025.4-4838?ï%Ù¾wÊgÀPú¹©çÀ:ê"ŒòÂÀ<²ÄÍúÊ6@µ·O,´?ý$ÞÚ5?Ï/®™[_?Ñ0ñd†½I?ýèú}	@@eò†ðŸ¿ã%)Ô½\¿ç濇iì-¿Ñ"…=l3¿æÒSŸd^Ï¿á&á¶hÝ9¿ïÿ«çy÷=UNASNone?ïēÀ°?t•è?×Ý&?J+:"Ôº?AÚæs%¿?zqe¼­H?sxŠ­¼?ï}CŽLˆ?'Ò"gŽ?JXhŒsä©?Zì|Þ'{Œ?	•äº"?±1ŒOoY?í‹žmvf?–6ü°í?'L`ìGœ?濁ø¶?°™€vÃÐ?'Ø–L#š ?îÛ`Ӕo?‡µaðQ*ê?XÆàðÔR?M9ì^ƒÁ?¡‰)›¿2~?‡……ÄiÀ½4FGL J0025.5-5936?Ü\«ªÆÆ+ÀL›â.]á]À:úŒð=ëÀ<bēBg"@äù~@±aCç¶]?ʾ=ö°¡?¯Ò_]ނ'?ãÁ¶¹eü@G¦(s<¿èºGúj"ɿᛃ´UÿåØ?\6a¼¿è¬x™nÑo¿ã(¥ߙX¿ç}YÇòryUNASNone?ïAéóË­Á?¢#¾¢n2Œ?PžM»[ŸÑ?VÍ/ðýb8?–¸ÜªÔŽ?¡š¹(Ò¨¡?ï~¶.ÈÅ?µ<ð†?G…™Ü$:Ü?Wì>ôXì{?ŽÚ°5Êó?Ž(NNòF?î'lº!F?'cp5Ö±Œ?v^Չ¯l?fÏü½)?ª½Y­¨™?כFÉé?îðÉ&ε?…ßXL!M?S±%;zðÙ?GÛÊL? b*C·=+?…îìÂyøÑ4FGL J0026.1-0732¿Ý§5t½'yÀQa 1ί%À;%sW±À< "€,á
@ fÏlå0œ?ý†»¦3ÛÐ?ÎS!¥—(Ñ?¶ cbPJ?ì7p¿°¯‹@rãºzå?íOKÝyn?Ÿj¿çdq>[°U¿¶Šùm¿¡¿ìô$)ªô5?â2ªw7oUNASNone?ïA^ËòÑ?'2‹OõzË?a½gÈ?Z>—LíØá?•³ŽÔµä´?«ŸN9D×?ïxómp—f?'Zqˆ˜ÜV?Q6è	Õ®F?ex'áse?œG¢ŸpŠ?#ÃÓ:k÷?핂(k~#?–A*g˜‡ã?ƒ¹Ôå0?wáó'?°ð7' 2=?"úåDq?î.ç–i?"nÔÌK?Ð?{§Ëêió¶?rîˆÀ­ç?©©X	L1?"{£Õ°w4FGL J0030.6+0539?íýò•oyœÀLiˁs2'À:5ÆTǏÀ;å¶BFÌm@&›–Ÿ@ßR@>´q?Àª"¾"y¿¨jԊ0p
?â¶Õ^ìŸ{@÷ç,Êc?ÍïRˆ¸ö¬¿è"NÖý¨7¿ìç,­'¿éÜp
¯,¿Àò§è;é¿ï÷íA·ZuUNASNone?ï'Ï"Ò?¡€ï?möý.}?pðúžˆv?"<
9—Ù? ï§7?ïÏ>üp¬?'*ù¤ÙdJ?J•V÷Y;?eCÚK¹~?Š"ÚÑnAz?ªàûŒ?éæ¼7žÍ?©òɽ§Šê?œ¢OQR?‹¼
BñK|?ÄÐÍŸaC?§ll'–ö†?ïya
ÝP­?¨ô8òÄ·?H7™4u#Ý?E!iå?!Ú²AI?gÐN"çk4FGL J0030.9-3618?îu…íⓀÀSõ¢œwškÀ;¹6‰)	À<꒽ÝEÁ@ ÷"	â­?ýºžavÙ?Ñ RÛÅ
;?™Émœ»	?͖z·]@΀×?ï_;#í?æë"²È?à
.A0÷Å¿â§Qa¿Ý1ð¥¿É°"‡äUNASNone?ïÀè.lû6?tæ5w­Š0?4ÌÅw"ñq?/èÅ"Y?~?r
Ç?twJ?.û-i?ŽŽæ9›?Evüjܒ{?c€±{¹3¶?‰Ãz†Üu?ŒôPé9Ç?î!t;º[?¢5´n?sÐøk+"?eÿ"tjšö?«‡B'æôç?‹úŠ´½òù?ï+ªKJ?ˆ¸g¸¿›?R'¸ÿÏ"]?Q^'Œž??™a›À;Å?‡Åz7º"4FGL J0031.0-2327?ÖÿiÜVqkÀUÃa@OÀ;ž7Åi+À=0ºö
³¸@]]àÛÍq?ùºÿèƒ?ÙÁ½|LØ?èžLa…V@
ù®º"e?þF a3÷¿ïÿãDÞVb?ïþ'AcL«?ƒ,ì6
qò¿âmSà§Ë¿í&ÕVß	æ¿ê«ßí;^UNASNone3FGL J0031.2-2320?é´o¸µ?¿gŠ[ɇ"?±ÈÍþÇC{?®Á³.ÀT?ÀIܙ¹Š?º!™ðӅ?ë¶C{?ûê–ïª?¨ë"v¸v?¸<¡Âµ?µØT]£ÓË?¹Â_¥v?æÅm¤ê?¡?®ºÏë»?ÀW[På½à?¤o|$ó?ĒîqC?¤ÕL¨bê-?í?ò[üÓò?¥…œ8Ô}?œÏ6z)?'}ëOœE?­™M>—ƒÓ?•–l¶CöÖ4FGL J0031.5-5648?ëø7ÈsÀN/Y‰ßÀ;0zW´ò»À<Ëo¤Ó‰@ A2û*?þˆåo®?ÌYO<(OT?¼\iãH;?ò@€"С@k–$ÅZ¿íYqýÌI¿Ùc"úÎg׿ۑÙüᨿà}ßÊÖS¿ÔNád‰l¿ïûs¾¾—*UNASNone?ïÏdÜÅ@¿?oÇÔNÜ:"?3@ÂÈõ†6?,—šnÏ|?w…pÐH?n÷|¹'A?﷝¦>"?"Ž"Ó}W?/‰¦>|…?ESÖ¾ÙÙ<?šoã¯}˜?ƒñ~-?îacVj$¼?Š ê2äß+?nëÒ|œRü?`z
<ò7?§û
q"ï?‰LOò«X«?ï{ÚQbº?v˜MƒX|?;~°?QÖÂ?2šk{'?»Àa?uûq«só4FGL J0032.3-5539?é–C	%SÞÀN á`؇ìÀ<åÏxÀ<ñ#¬­r"@$ïW'.B3?õhB>hñ[?×ñ¿Ë\ŠE?º	Þ%9Ë?ÛB¾@—õ«@#°Ó@¿êð8ÂiF–¿ïˆ!!7Þ?ëjé]Q>â¿ÄGûa@b¿ïéØÖ+?ïâ±pOô4UNASNone?ï­
¡§—m?‰tWú_¯q?6H)àëP?AšÄݘÁ\?"
-TËl?‰îßDñ?ïh^j|¾?´rŠ¿3¨?Q^dV9àB?k«ïªà¿^?'ÞLk*A?œ'Pwùæ?ì"
l×»d?£+$'/Eo?€êâÞQ£?|ïß÷?¹B8=x¨?¢ßÔW1?ë´M~´&°?³ôªÛ—ZI?U&v†›ô?e~¬`Ð?Á}"/
?´ø"QÅG4FGL J0034.6+6438¿ÇNÄ:œ+?ý7ú'ص8À9›[ÖÀk•À;hb{[@<©ÏÜ@ø{,Ç?Ã؞<@£?ÄW'afÍ?@yà{Ö:4@‡å‹_š?ïöòl¬Ò¿ÍkàÊÆ¿æٚpY.o¿æ
ë­òí¿å[LVñ¿ïÿöµšUNASNone?Ùë",UX?Á×'ÂÅ?¡Nµó;q?š>"¦Ü?áõK
Ã%=?ƒ÷]Ö¼?Ð+õ…Šž"?Ä¡Gà¹qÊ?­aÓѪž?°=~hð¾?æè Ü?ÅßGÅuŽ)?×6Ø}b?°HüMeIk?³¬ªRsy?",ü!ƒ}?áò~]÷J?®õ
šhh?Ô>;å­ú?¡¹ožØ?¸@eh:a?—ï'È»²Œ?âØÞ Æ!·?¢¿Žáë¢4FGL J0035.2-1739?ïôrp_älÀSôÏþ°t§À;–…AÂÀ<Ù¥o±"@!\Ç
Àù/?úËg<O;§?ÒßÝ5¥©?´>ïÔäžP?äYaϨÊ?ïœ,@¥·Š?ï÷òµ"¡ã¿ë¯8gOšr¿ÛöÀ›æûÍ¿Çÿfèle"¿à­ëá$
¿ÑGã¤)ÀnUNASNone?ïÕÐ`Ëf|?pý¯h-Ój?éE'Ó?Ü=%²ÿ&?t˜Àô«¦?pÙÐ歇Ï?ï
p¿2!}?¡ó",—I?j¬Zwœ¼?‡1±êƒÄ(?šü\ÊÈ>u?žÊMx`t[?í܇ªÞ{I?'rdbg?t
š[74?u'nfÚ?¯µÒŒä†?'š§ãÁ7?ê7òï1Py?«
ù SI?w9v¿Ì?pÍôëÕ5?Æfh<Z#?«0K÷õ«4FGL J0037.2-2653?Ўl¸Ì ÀUµI''>À;¡éhäÅèÀ<¨,¤£¸×@"ðE¢Ìs?ì>vþdŽ?äy(_ð€†?ïäkß÷÷É?ù–wƒÅ?ýû†5ä"h?ïó°0´Ó²¿äÍp@"Õg¿ß{W#ÓCß¿ØÇáÖt@¿ïÿÆTǏ¿Í¥˜¯cÛUNASNone?ï &Qô-ö?¥ºkwV ?nRм¬Ï?pIAÔuO½?˜0Ý-¢«œ?¤Šiº»7µ?íõҀÍ´?¸?Þ;t Q?ˆg3ú`?¤æJ£'?ª‰&g/?³v3‰Rî'?ë?'ї?¢-eä?¦?0\+:¾?'K¬TŽ—?ºãßqãÕì?tݨ°ã³?èiŽëO?½'Ñ·6að?emºI?q8­k*?Î]jFË?½¤\‡O	4FGL J0039.1+6257¿á¤¼"ÙÛ?¿4GÛ5ñ)À9Xº'Gm}À;ß|ÊUú@oeÉÞZê?þ|óÁ-\Z?¾Í³ýsß?áú|2€…Ì@ Üa•FN@åÄè4Ý¿áP"G!ý¿Ú祖'R¿ÈëJw—¿äÉ"=—*¿ï6©Àd¿í ˆ JxIUNASNone3FGL J0039.3+6256?p´03©¼?iד š›?î|ʹo?¤Éc'¦
´?¦ÙBH"Ú?£Ö™MN×?‹ŠWËãN?•ÔËaÛÅl?â"î$ô÷?ΆzæóƒÉ?ÚÝÓ5¶ø?Î"&l5^?™KÅ@›Û?"*'[à‰?ë×j1H?¡T1°k?ºôû^Nûj?ã%oøg?Ÿå$Š²tÓ?ƒŒ4!´žï?åf߬ÿ‰?³jª}ɀ?Óèß÷úÙ¢?²gcH©ï4FGL J0039.7+4203?ÕÒ³'À4Áæ>ŽÀ;4ebZhÀ<yÏÛu<@È8ªky@ãp¥"‰g?Æ~ÈÈ[N?—Œ|ù?Ò¤_۲÷@)N^³¿Ûè®àR»¿ÊCBtï–%¿êbÙð!¿áîmØJ¯¿à?ûÞ]Bü¿ðUNASNone?ï"-Q·E"?"rÈÜbìÈ?PîL¡WÚ?FÈ5r[Ì?ŒÖáþÅg?ƒï˜åÁ	æ?Œ'x?ˆ"ÅBÅ?9mäYf×¢?L˜'[ãÖÐ?Šˆ-¸ÖÄÂ?‡ñ´½¥€?î
"&xž?•*k¥õZ?|g¯Ï'É?kú­W€-?«ÐéC¸í?ŽL¾ãP4E?ï$fº"ѽ?|I-[J³?\Jð\¤?L8	ð$\?™®‡þ?|—Þ%4FGL J0040.2-2725?F¨'sÀUßµà÷üüÀ;BH­î»4À<|ڀ·@jõ['@‡wÞ]îÉ?Å^j™{炿ª Xz•rn?ãö«ù®r?ùÜÚ
Òüg?ïÿýaw¿êÖa +n™¿æƲ×XA
¿Ú~YÝA¿ïÿã_¶Hý¿µ	-%RUNASNone?ï¨/`Ã>? 
úÝq?FЅ¾Ú/Û?Q® 9³|«?"‡sJm?Ÿ—›™—ž?îwY¼?Õ?´B¤ªŠ?tn…z—Õì?' ÆQäæ?¦)´éø?²E9ý"?í†ñŸJV?˜½:`¸#`?'MvR?w'Ðd]L°?±–R£ã ø?—t[ZZÜf?í"zAçÂ?ôF"±.É?…ºp7o'?z]ëíu-?´dŽ-‰Ô?œ{Ðð4FGL J0040.7-7157¿éÐsa˜TÀF'³¿µÀ:ëHɝmÀ<±'¥‰'å@ ¥×Û?ý%=§*|?Ì&ÝåMø?ÕI7º@fÚå"Cï?ùš¥]G.?ä)€,
¿ïA["Ì´?é±Ç2ŠA¿áPÍ ¿æh›ÊÌA¿äÀ;#Â|èUNASNone?ís–O‡´?©èWðGtµ?xöy+çè&?s°òG­©?²Óåô}CÞ?©ZÛì8S?ëñô#r×?»P¡ô†fž?›:ț¦?¦¥ÚqÊ?¹¯ÐG'Bd?µœù̉ù?ë¹·o\Žï?¡Ï½‡°µ?ú…cÃ?u3ÐQlT?ºñEãØo–?£¿OMnì?æjÄ"Öå?±zÂ;"õ?¦5šœn?žêUE¸(W?ÐcĀöþ¨?°'ÔGK
4FGL J0045.8-1324¿àÉ+n)¨ÀS
¥¹bŒ½À;§/F>¨²À<ò×;»—ñ@ rj Z=Ž?è×ÄýËrZ?ñ')bÏÙ?ì/"YÒÚ?úÀ?ö@Wÿ÷òjk¿î'ËâA(>?ïþCÒ½§–¿ìCʟöÕà?Æ#ˆIe$¿æÅ&p­¿ïþz#²Œ°UNASNone?ïz"<É:á?Œ?c¤X‹Ç?pš8@.«é?p-"Ö^Ø'?‰*T­™ñ?‰‰gë_;?ïiçò"jS?œ|&zw?bÉ3ºßO
?"Âuœ´|?iÛ66ËÃ?—d¶! ô?ìñXMŒÉ:?›|n8õz?'"<F‰?…ãa<S†9?³Ô.'?—wx·CÅ?îüã9u­?—A\x^I?@þŠÙº?e3׏҇?ŸÛ˜˜S˜?–Þ NÑ©4FGL J0045.9-2021?áÔ?cSrªÀTÇƧÀ;2/Ú¹šÀ<Ƨ?tŠ@ 5jE8?þõÄ}î?Èüí¦â'?¦GáýÛ9?áíÜçÍS@‡
íC峿îåNCZ?ïô¬ç#¿ânZ†^Sr¿àL0Z:ß¿Ô&2™°?οêT^/
ZUNASNone?ïÕ.&?tÏjXèþa?D`­tú??q• d‡†?{基=ÌS?sêÁ·ÐJv?ïº<ÀRð›?…Kò[U?/­A{úgF?F•¹Êÿ?€òåSïÇ?"¯o]i¥Ÿ?îKT"¨eß?‹¤¯0ÇÄ?oJXÚ
]R?Yp\åút?©V'ØÌ-?Š…6µYw	?+&zu?t§£9œŽÃ?I=øŠ}{1?A—#œÑÙz?Œˆ­¹‹V?tjP*4FGL J0046.7-7048¿Ô®×˜F¢ÀG'ž@ÈG,À;œ¥R4€À<ÒÆ»:Ô@Ӑš—@¸j$aY?ÇÖÎûtU¿¨ÍÆᕦ?â³þÕ]•@¢Äþ¢1ï¿ïü]Ä?ït£`Aß¿çÄyA¿àèõW/'¾¿ïþ5Å´ª—?ïöÇ<jšUNASNone?ïÔo"?s +K÷²?Wîä8Qv?VÜþkŽ:.?o˜ðÈkÌ!?p;ôõq¥ý?ï,¿ÏШ?–©0è{"?UÞ¡#¯?iPT›i¢à?™
ÿ;ØÕ?"¯Œí…‡?í4ÆÀh"ú?š€°P¢wø?‰†àbÐÛ?€h'óȹ}?³(íða]/?—¢ô…oW?î¬;©6?Ö Àô4‰?uˆßsJ7?o+{†íí?¢‹)~;õˆ?ÁËN4FGL J0048.6-6347¿Ñ¤L`*ãÀJªÄÑ¢À:ÇK^£#†À<Çdl'"Ó@)?ý<Aÿ~Ñ?ÇÎÔcïé‡?ÚèŸ%ʔä@¦Kaþ"@.ï\ڗ¿ð?ïÿÿ)@k*¿ÙHÅ×Eî¿ä¿Ä}îB¿èÙXáÃ~ð¿ïû²]µ½½UNASNone3FGL J0048.1-6343?äfÀ…2±?ÅàdâƒÊ?х"LoÑ?Â툌†?¹fxÊ&w?½ø%`ó?婃sí%?Ê~t!?Å0²ö‰Œ?ÄYæ¹I(r?ÆÀ—?9Áá?ÀDæ5©ú?×"¯)Éç?´ÞxÿÇí?ßeÀä
Ty?¶…Œ²rJ"?ÂðdٗÃ??¤ª•Ÿ&€V?é2Ê_‡Â:?¨bÏK9I?¸çƒ#ñ?¢eœ]æn?¾Uŀý?ž"t0þóâ4FGL J0052.1+6444¿ìB´iót?ýíözE@À9y\–$À;Xfêð¤B@•ËÊï'@è‰͟[?ƪH(äj?Ñ-P›#•@Ý ×ç?öؤ^™"d¿Ô=ՃT³¶?éµ{âÏm'¿ß§›š¥³-¿ên¶—b&¿ëRæ÷ñ=Å¿ïݥ̈́'±UNASNone3FGL J0051.6+6445?œ`½£á?–Õí[«ñO?˜ëÊIŒ\?™ó4ù¸ÆÇ?îU›Àž;w?¤È>ÁÞ?·‡kJ þ?¸Êyâ\Qã?ÐÚ%kÃ;?Çjø%«f?ä¢ø
C?ɍêLr†?Ç40m_˜7?¥¤7QÇß?Ã;­bZ¯p? ™Ÿ\˜ñV?ådŒn?ªsæçk ç?Áîñ4'ò? v,bìï'?Ñ|'Å"t?±JÚ>l?âÝÂàè¡y?²mEF¢ÁA4FGL J0054.4-1503?浿~ýÙWÀSz îõÀ;íNäHÀ=]¹ïzw@!'|`Â8?ôÈ͙{f©?âf~x+
?êT•ƒŠcœ@
ŠBä?üù'ó¸¿ïÔwéR?ï}WÎÂ?ïéR‹¾?Ò¹,;È-+¿á‹Y/F>©¿ïøu'ST;UNASNone?îŒEˆÒÛ?³'f¢'?'Õ¹[†ç?‡¸²A£—?¢Š]P¬p‹?³_dOn?î{8‹xëæ?±™yz÷I?†u¢!—ò?¡D{é)ÏE?¢¯Ã(ۖ?¨¿ìò?ëÅ«e{üÓ?£¢&OCå?¢ÐS	Æ°?"dhÑýõ»?¸j{O=
?­Ý1dé'?í@ð"?¦¸Cõ͈?€þÅ|h?€Þ·zlD?³ö@&?·ª?¦t]X¢‡4FGL J0055.7+4507¿Ö—µqo¯À1½šA_EáÀ;ùÕm…>™À<ý3þ4Må@"¯e3?÷(ÄDhÝ?ß÷×\È­Ù?æS"ÛÈ@a.á"Úî@$m/ƒPW?ïÎT 鄓¿ïÿûÞ]Bü?ïÿ)vP¿ÍkØUÁþh¿Ì¼Õ~@"¿åÓ6þï´®UNASNone?î
(N­9"?©ÙGå÷›?€d·6$*Ü? (á%?«MG£\?¨M"ïC?ív{8£?¹¤y¡¯<°?ˆëipdÐÕ? ÅkrÙLø?±.¹ÒàË?¶–7,ƽ?ëÈE®½¡R?£ŸÕÛÉz?»}òØÑ?'¶Žä2í?½Žó
\ï¿?¢epQß_?è†ws?p
?³s}aOÊÅ?xÐyH¤Š%?wHÁîÏk-?Ížh½†?³…·9>4FGL J0057.5+6814¿áð´<ÕjÍ@{ÔÝ<†™À:aGzÕÀ;'Ö*'ò@4¥Ó
ه@ºNz·VC?΃†d9»?¥n…ž?ßiÈñuù@¯>dÐÂ?Á+¡C‡Z¿å­VŸôÒz¿ëŸH˒:¿åTê"H)d¿ëŸ¤À¿"j?µ§\лnÖUNASNone?ÆO	óÓÒ?¸>Ô*5/Ÿ?"tp"«?Žžù¿,?éȚŸno?¹©Ìt§?Þ´¢[ça=?ÈýÿþË?•Sf¡«}G?¡¾V ¿U½?ßö'9ýæî?ÆÝ
Ök&?ÝþyÎgÌË?±bˆH—?­GÔó-n?oŜQA?ÞX‹"6͇?°£"–{…"?ä;E"
 9?­`DœPË?‡Ï»ë×l¾?tèû¥¯?ÖÊ÷܆'?­ðóYT<4FGL J0057.9+6326¿Ú¦Prß?ânù´
3À:{›eK´3À<-yøêb	@"óXˆØ+P?õ~€Ǒ$?̾ywæž?ÌÂy6͜€?ùۑÁ^Á@pUÚ'(c¿æòI~N9Ÿ¿êÊE3÷Å¿æÅp'Iü¿ÔSÈ
L4¿×Á'è|U¼?´°bÞÇv!UNASNone?Þ>Âäé?Æ3ô}Põ?q®ìdc^…?j&xgl
Ÿ?àÏÅÄĵ?Æ%D°[?ÆOò«?Æø.HëìA?t';oª!?"dJ…2ä­?êD
ßuÉ?Æþ̯hó?ç*W«
ä¡?­ÅXË ˜¾?"ˆ+d‹ð+?€|UØüZ?ÐrÍó¡wº?¬!jr–í?äG%*3?¸We«"s?tªÌ‰ÓìG?sߤ2ˆ"ù?×:ƒ®[é?¸‰«%ûHm4FGL J0058.1+6915¿àþoU½¯@–tŽGVÀ:AVZ¨WÀ;¶o×ÿ/ö@ÊæØf³é@˜±¨ó?Ê$²;üÛ]?Áiànj?ó0¥i±t'@¥Ðȯܧ?ï,pk¢æI¿æÌs 3&H¿åM÷¤ç«u¿évØa´P¿ïÿáåÔ?ïþø™q¥UNASNone?é%òüä¸?¸ÂQÒ2š?ŽçjŸÓ?ŒM‹¶5×?Ɇõ™>{B?¸B6ÌÌþ?Üq:~¯"ƒ?Ë؉}¹?¥öÏ(HÅ ?¯%C¾ˆZc?àgõÎ#©m?ÊÕ6»R?âϤłh?°ká€Ý÷?®N89?'ÑÄöJãF?֖ït´º-?­¼aQ,òØ?á™I°¥L?±ÀËËÅ?§{ÓÏ}œ?"ß¿¨âؘ?ÙÞzò¯u?±SKŸg4FGL J0058.3-4603¿æ£"K™ÀQÁqKœ¶…À;µÀ_@˜À=BûÅ@ô*û×&m?ÿZÊ¡yaì?Ú¢w{?© ÷œY<‡?ÊYƒ©î%@YÅM~¹?ïaì¹ÒE¿ëlÎàM]+¿Î	m&žû-¿ÜSa[ºà¿åG®záH¿¬U½KÐcUNASNone?ïš1‹MK?'Û'!•N?9ôܘ§k?;ž8FÝ×ø?ˆ£öGçý±?'š~Zu¤±?ï—Ïð—?´É_¿Þˆ?Cš'''0?YÝwJ5ˆŽ?ˆÒ£Ñ%å?‹ýCª©£?íÉ´r™?–§é0mSW?owN'%«"?nÆ,²¶¬o?°¶¡öªV©?–SVÅì?Œ‰$?v§âÇÍ?$Aà%E?"ËÉ»[3?‹
xe"?vTpØï4FGL J0059.4-5654?äÐó¹†ÛÀN°ËæÀ9¹Â^´Á=À<êAQÚ@vr€ó@¢ÈY …F?³K¯ÁN>|?É·¾]HZ@Ú­Å@§Ó"ý0¿Ê]%Ÿ÷¬Ÿ¿á¬M P¿ænij&å¿ê–a¡Çæ¿ì6ÎÉ&O¿ïûÛxa:­UNASNone3FGL J0059.1-5701?îï"#-?£F;ºc³Å?¥
™~÷ºh?ž&§+ó(…?"goÌ%y?Ö˜°Å!ê?î¨IR‹'?«­WÓP0Ä?'ï€Î¹›? ¬œi"Hÿ? ÂK7(à?¡j›âôeé?혜åµ!?£Š.¡6§ø?¥àçž??˜³X~¸R?ª&öP½º?—€w":¯?íò÷rŠD†?ŠB†àÙ?'œ(­¡Åš?}_
ÑÁûñ?¨t€ŠÔØ?Œ£ÅDTÉ4FGL J0102.0-6240?çk]QûÜkÀK3¡fµÀ;eTÑél@À<à£ó¯5@ N:¶?ý»ed®?Ët˜Ù*S;?¸½ÔakªÉ?ðuøÅyu@*AeûÝ\?ìö—€º¦?ÔüÍÛëx´¿Ú}âïN¿ÚÁ1æ,¿æÕ)' ¿É :Š¿âUNASNone?ﷇÀúÉ?tM#Zx–?<~±øyÇ?0¢ÃùÄe»?=ÉÚ1‰ü?sé'µê?ï™MŸk¦?†ÞîJ]?:³5=ÝV?KçŽü+ÍÀ?ˆÖþ{Kì?†'¹ìjz"?îfݐŸÛ–?Š×d¦èÚ"?kRqmùœÒ?Y†ß0M?§Üÿß"¬á?‰œ‹àÍ?ï1¢*9'?€ª²œjçg?b«FE»_?Tˆìß=¨?—vC'ö?€š}ÛL4FGL J0102.1+4458?ç¹+¿îºÀ1ܬ¯öÓ1À;@e+ÓÃÀ<®Ó5œš@ )çJ?í)•€r+?ݾ¬
9¤f?ëìjŒeÔp@<¥¢¼@¡¶É€<%¿ï£'Á¹m?áÎϦ›àœ¿éçzBfV÷¿§k®yÐ{ƒ¿âXxgꍿïús™TÐ<UNASNone3FGL J0102.1+4458?ïAüh<f?¥ øˆboÎ?yA·"*t—?†—š%æ |?'pMÖ? –á'È
É?îÇQ"¯¶=?¬AraÍ<x?v‡	w5?×ÿ€»Æ? ¹÷ÓÕ¬	?©
—°?í*$T¨?šC1úÂ<¶?'‹UR_?ƒõɌXu?²0Üjû?•áe…2>?í5¶<ÉEu?¤‡'¦²Î?qž*Îìrv?x|ìѲYï?µ8klÇ
5?¤k(m¤oì4FGL J0102.3+1000¿ÄA1RÀJaä¼­šØÀ:µ¸•Þ#6À<aÁLf
@ œ¢»×1*?ùÙú—á2µ?Ò[ÈRèÛ?Ú³ô#Rë_@˜Cæߞ?ýqÆ^s¨Ä¿Û®ž#/—¿ïÄÜ"«%³?íûÀ«+g¿Ò†É]VF¿æ4½vît¿ä íìEzUNASNone?ìõqø¦¹þ?®SMB#?ÄÝVÛ?|;¢"Ÿô?¶ßÿl¸?¬Íü4Õ?íÍ¿Ù´‰?°òK5°ù?"¼'EF¿?'ý:Q}í?®º1e«?«–દôy?êR{›r‹þ?© DÍßùl?žfsEė?Nâñh/?ÂéC)"·q?¦@qª4õ²?æÓP¢—…?±Ü"ƒ:ôR?ŠÄKæ†|?ƒAä?у<[¡@Ã?²y³B¹a4FGL J0104.6-0818?à$õº_jÀQ»<`ŸÀ;	7·&rÀ<ƒM#ŸA@/x›æ@¡Ñv€?Ö ¡`7x<?µ¶|~UÆ[?àˆÅ †l@½6	Í¿­g:f¿í»Ó`Þj¿Âe?	U>¿äÉùHUÚ'¿ïÿîͨ"ß?ïž^z^ÁUNASNone?îï$t:K£?ž
‡Ô£½?Xã"V#­T?WÃ(‡²? Fœ!ª(h?ž^æµ­?ïm¥Ê2 ;?"¿ÊÞ?S¥ü{ƒ»?f¶÷ÒËwú?'æñó¼é?'ß´\_Ë:?íz̵0¤?"ÉÿöŽ[9?'[ã¨??…>õ:'M?¯ÜåBØÖ9?U4+"{?ï0½¤.K?ƒëkáÁ?Døé"ê8D?@˜èAðþf?™@"-•$á?ƒ¯µÑïv4FGL J0106.1+1131¿ïÐLX?©†ÀI–áïsÀÂÀ;ez¤£À<ºÓø:9@ [ž·:¿?ý$™ù;?Ò;9\B 6?ÐX9™…x?ùO¡(TH@ç`Õ®?ë<7Þé"é¿ïþôœõn­?ïóeRj0 ¿èä‡Ôu7»¿Æek"£'¿ðUNASNone?ï˜|ºÖ²?''î8šÆ-?Gɼí%w?M¡ëæ?ˆp®ª?'hTò?ï¨ÄnØÙ?ž€2'+°?_œêYsQ/?w<‹x¸ë	?›̍¯³?›g½LŽ?ìI•€´?¡^ÿ}po¬?ƒGtö·Åœ?z/èe¶n?¹ŒÄ¸U¯?¡²š"Ôþ?î[³S
	¬?—Ócì 
ß?CÜY!žº?GõWôŠ?©õYjöÞÉ?— ""Ó\4FGL J0112.0+3442¿ÞU¸€†ðlÀ;úÞ]	À;/6oþ•À<µS,;d@Q#RŸÊ?ÿ×_f˜?ÙüxŒØ"?Þáp}–ƒ»?üÞΌÀmC@
?ىʿî´¡'¢?クAûM¿ÞÙ§{¯xÔ¿ä ‹Ær?¸¿ïÿ«çy÷=?ïüK_ÏÉVUNASNone?ïF0bìê?¨Òd?'"_.βý?€ð—å:Eš?‹ßˆ)¶q?‡Ñ<â¾&?íõÍ
É?v?­ÿ°	´?œ?*¿"ìH‡?*u$p¹?¬X>0ö{?ªqý̱2?ê"þ‹aj²?£ÇŠæÌö?°¡H¼Ùˆ<?–½Í«™')?º¶Âè"1?›j o)?î_­ë…ºð?'›E3B?~€/ÌÒ?tmÞcmT?¦5N
ç?' -ï:4FGL J0115.4-2917¿á²bigßÀUvÈ´9XÀ;‡ÚÙÖÀ<äÔÉ'@ µQù#?ûûI·Ùö?Ֆ¬Ÿ…ÁË?Âß#¼r·ƒ?ðZ%Ðt!@Û¨!Ç¥ñ¿ïÿC*!<?ïéÿºùf¿çÀèÞ%d¾¿·½WÓ{"¿ÔÝ[û©Y*¿èÏ^bùUNASNone?ïÇÔF†²?r¥Wµ—>ë?<gºá`?5*ÖT÷Í?zUÆL¹øè?r gˆþ?ï°oP¤Õ?‰µ¤ݑ?4Õ0ÝBå?M¯]˜À	î?ƒ=ƒCх?ˆ·pÒþ!?î"­Š ?¿2Mó41?n>Q>Bf1?Xð®
:?¬ƒÐ#/ ?ŽÆ+â3j!?ïhZÍ蛟?|ù'q?? ´h$?<£ýÚ	?'vpiº|?|¾Kè Ø4FGL J0116.8+6914?ì{b]±ûª@ì !sOÀ:Eûg¿,À;Ó2ӑâì@®Gp­@=Û	íÀ?Ò`¡üi?éÃãŸw),@Š˜í¢/j?ôå~I‡¿áWR'ú¿ÞHTbWãí¿éÜG^cb¦¿ïýÅÞFî¿ë~Ïu¿â©¬ ÚÁUNASNone3FGL J0116.8+6913?Ç	¨z8
?Á4¸+ír?Ô¦Xè"+?ȕ—#®?à4*im(h?Ê;b«Ò?¸¡Ê=ÿoX?À—Þ2YC?áF%³ž?ЈÕä¶?×K"R4¼î?ËyÕ¥'\?Óþècè$L?®¬e'ßÄh?ÔÓ6Ózø?¯È›¹¢·J?×-˜eD`¼?±¯Zf?¡}X—¤%?Š™"üg?äñ
áPÑ?¹*pËn]?Óî9*iÙ?·ŒþVÏ4FGL J0118.3-6008?¥´Šê1ëÀLUA [ÀÀ;Ëô_¹À<Üò@úœ@¹±Y¤·@&Š"lXï?ʇSÆы#?Ǖb¨@ÑV?ü°Í'eŸ—@m-Dܨã¿ï"Eg]Ñ?ïÆlËÛ5E¿áÅ|vs#ä¿àހ("Y¿êͶ±Æa¿ïÿ¼®q—óUNASNone?ïäÞþ†Xò?fÇ_ŸpË?PýÃÜø+?R%ŸÉ>)?b¢‹+˜?`öAS?ïÄÜ@ ã*?`ëõŒ…?1YS«îeb?I3'£áä?||Jtτ€?€™DQBK?î¶LWQúR?‰ü&ú!Õ?~ùJ$fއ?xaý΀ʯ? ¼FS~þ?"º%ø[šø?ïÅ$©Žèì?cQò胆m?Tê⃙Ì"?DÿP£*}Þ?x2ò—¥/?a¸<mQn°4FGL J0120.1+0505¿Þ»¥ ûÀL…£~õ©À;1bZh+cÀ<aG¾Ûr'@Uë²;|@ÿí¦a(9?Äõ¹NjÇ¿¸¼öëÚ.?òÑ8×·âZ@¨«B8‰´¿Á1³VY(¿íáqŸ¿á_ã*cǿ⼫™Ÿ¿çª£	"¾¿ïÿ¤DîUNASNone?ï ï×Ìõ)?šôÀú˜<?f¯ý¨¨ä?b™:»U»?™dìEÏ?š`Pë$?ïYpÆ&Â?–{×e-!Ü?RœtL'ØT?k²ã†íƒ?"¨øqú=?•äRÚ?í´m"&'?"uŸÝ\:R?|–$çüé?m¦Eþu?°"1_
m?"G[†´Áœ?î2¹€5©^?'Ë$äwEu?ažºýOâ?Xuqžt?«º|[e• ?'tEÈ×õ4FGL J0120.2-7944?îÚÑ4€kÀB¦>-b9À:ÛWvšÙÀ<-"¶³…Ô@L>7±@®åD'×?ÃЀ¶sÄô¿·gɽέ"?øʶ!œÁ@BÏÁ+?ïÖ%œq»¿ê>
A¢a¿¿äè%þÂ=R¿écÑÌk¿ÊÉ>!ù¤ò¿ã+ÕÁh¼UNASNone?î…þN£†˜?°HÿŽ%?]U&-0¨?\Wn®?¦µqä[þ?¯Û ˜RT?ïï}Èc=?¢¨›)Ä·Y?^[ävrb?u~pò}ÿ?ÜQþü1=? þ®³ò?쵗9êw? hØYB|?ó\åhV?q«Ô#Öâ?¸ڛCœ'?ŸHž«)1?ïµ¹àÇ?ˆÑ|?À1…?J܉{¹¦?GXq¦^ˆ)?›Òdx ž­?ˆdjÌ
4FGL J0122.4+1034¿ï¤ªUáVÀIÇ:Þ"_¦À;—KÔèëÀ<È[Q_n%@"5Ï`ûÃZ?÷{Ãà•®?ÔÔÈ#š¹Õ?Ôwã¼R?ÿC;¾òïv@aƒ~ûÉ¿ë-Óî'¿ïÿÿ>¹ú?ïÿç@ìYZ?Ô1ÄPÈÅ¿Ýbí`>¿ÖöçþV‡¡UNASNone?ï¢ÕD	?ƒÇÍE0ì?C»BS¥A?C2mVÇ)?†ö	"¢m?ƒ<÷¹hUq?ïZwmhÐ?'¡c8•Üã?L2Ém+¡?_üÐcÇS?"Ð8¼³¼'?'‰{8›?ì»g¦îµË? W"i#ž‰?~'gÆWmÊ?qøúN?¸<œL$ÚÌ?Ÿœò`	´'?îªÛ¥°É?š÷W@&ØÑ?B"ÉwÊd^?A´+júM?­êÿÅÉÔ?šíDÚ Yq4FGL J0125.3+6820?í|q+Ö@³çÑ5ZÀ9ÛîùûÀ;x¡L'H@¥§Yޙ@´hqH?ÓL.!%"?Ðü^ØP@¼½‹j@&¼<
L?ïÙº`ú?ÎGŸ{ÛË¿ê×2K¬¦½¿åÁ'¶ÿ.¿èЩôg¿ïüuÁù	AUNASNone?áÓö_Tg‹?ÅÎiBj"?Ñÿ(¥Ÿ5?Åk(e
sE?Æ¢(1c#h?¼"
ê4i?È2G:€0~?ÀÞj
×q?ʛLõ·?Äé¢û5w.?ãLšóòÙ?Æ=ز#D?ԗµ[L_?­"Dü¤ï?Ãåû¦ó$?¦gÄû™›Á?àºò;•'‡?¯˜ÙfÈb?ÕÍ×L?¯ä1Æ?Ïf)˜3´?¶üJç‰uN?Úbg̚?¶Æªv_\)4FGL J0125.9-6303?àn\XèÆËÀJÐ\
V›À;D}¿H€À<Þ\)̂$@¡·â@ǧ¡š?Æ®^øˆèF?•ECV1?ѧa5úä@•èÞ%?샮uɱ¿â/-êôÖ¿è"·õ¥3+¿ÜCÄûÈõ¿å Ž¶È¥¿ÝVÁÃ.hsUNASNone?ïS°Xx"z?" ãV"—'?[õAfc?UÏÅú¡R?"Ê à…J–?"&gò[¯?ïyx)W¤?Œ=•ÑæÛ?C¹ù¢sÍ?S¸úù>9?4}>l}?‹$­À\¾?î¨cN¾?Ù'Së©?v憔Ÿ	Ø?cüë-Þa?«ˆ¨ü·2Ý? *Çt?ï_bxj=N?u>¿418@?b3=¶!?OêηB¨…?'Ñʏ°Ÿ?tž&µf4FGL J0126.3-6746¿ëp\BpïÀHJä)à¤À<D'À=-®Õߛ@!óhbêÛÖ?÷Æ5µ?ÚZâ9E›ì?҆êCM?÷ĞDú?û/,xƒõC¿ïþ…A¿êvjXŠÜ?ïûÚÂXÖ?À{ÝÆðú¿íƒ>Ò£¦?è	K¾DsÍUNASNone?ïjš3BÉ?—|G+Ã	j?XÅK—ž'?WhݯM'Ó?›†ZôÞ-?–/²?ïU&»"œ?œ¼ø"\Éø?`¬{%t?sbÕAC¦¥?¿ËÃìI?š]8$Á¿?ëç´E§'Ç? ´hò? |¿
Šë?'WÄÕ=î?¸ƒþM}ü?›!FŠ› á?íÊm*Ðk×?ž‰…uo>K?Z´ŽõÁ1?\iâì·	·?±AÄqpÊB?žMŸiR)4FGL J0126.8+2412?Õp†c9"ÓÀBú€If{_À:4ÿ—$tTÀ<EÔº.@£øÿ%@ƒCÿF?¼®î?Ž5b¿~áè÷¤<?³ðëºù'@êt¼•r¿ß^E"^ǿ䢅›µÓŒ¿èLÒJ»¿ì(S 8"¬¿Ò`P'yl~¿ïþÁÁÖυUNASNone?ïò>sÌ7~?i>ÊÆó]Ã??R8½ISÄ?fæXUM?S®Š8>¯\?Wy"WrgJ?ï¿ü9J°2?"
ŠÙÁõÇ?'HècÎ}Œ?I…EéFj?Gœ‰s?ƒLÞfÜö?îêk~I[O?‰kx™$?fb
{§?XÉ u'Œ?Ÿâcõ…5\?ˆÀ'–ùÔ?ïëéµêÄ
?Q@º«?"š5*
m?tä7Š%¥?bì¦Ä)T¶?P² L84FGL J0128.1+7542?íEò®fbé@)ÿ]5e<›À;,$8Äl¬À<žÏœŠå¢@W­~'ù@cYÿOÖØ?؉$Vv"?îš#A΁ƒ@þÚH¶R@ݲ"L*{¿ï‹oÀbV?ïâù)L)¤¿Ü¤K8ãv\¿í8"†<Ń¿ïþ¯çÜô?íHúåäËÇUNASNone?äL[$méÙ?ÈÇq  ü?Å­Ž€mÁ?À,Î-?É!íÛ<Ù?üã¿?Û‹þ?ÎòŒèÇ/?Úñeü®ƒ?ύÊÿ'Ïž?ž	ъü?Àÿ—?⬵Tã§?±5p–œ¯õ?ÈLÛ®U¶?©—ì¢Gð?Í
|­?¨³\àp?Þìv²~q?ºÄ§"çÏ?ÙäÓ«í±?¼ØäaÑ ?¼ºÖˆAÜ?¦µzÈÇ#4FGL J0131.7-5346?àw½FÀO*êt}€^À:¿¾Ô¼…WÀ<µâ;ÉÚª@œ,Œ@6&˜ðý?Ñï ´«m×?ќã›EkD?ú:¹¤ÑÜ@×'n®ß¿ÕLýԺؿß]"Y¿ÜYãÜþ¿éâç¡'û¿é,Š'O{¿ 'ðpUNASNone3FGL J0132.1-5340?ìeɞ'-ä?°@"*ëT6?'›ž¢9ßc?€<zo?º~?7'Tì?¯Jw½Ë9?ï3~?œ»wæqù³?i%¾¡IC!?vì\ޑãg?›÷Á¼ô¤?™®n÷7Å?ë•Q|'å?¢]h›XÞ ?¥ê´L,(?"Ù3qÎÚ?¸`øø€<?™è°®õ°s?î"á†ñ¦Ò?ŒkŽÈÏ<Ò?u1L|ÑÌ°?hæÎæmÐ?¥¾KYV?ŠÇàí€M4FGL J0132.1-0956¿ïäê{^pÀQ"KâCÀ:>_ïSàÀ<]o`
+Ó@¯Ûbç«Ë@'¤:Œ?²äôQ ?Ô.;&Ǖ@TbeOåñ@	šhÓ(0¡¿×Ŕ~ýŒ¿åŒqȚ8%¿ì†ƒý¦"¿éS>Ïu¿îáGB´°v¿ïóímVD°UNASNone?ïs£e,?•»®'›Ë?{à
RÀó?y¿T-^?…'3}§˜é?'hNtÔb?îtéíLç?³'¦…¿Ó÷?Žq'WDnÌ?¡ŽÒ{W~?§ÜPËZÕ?ªðRV}Íz?두e¦b?¤Óփœø`?ª/˜Å"6?˜!(ï¯>?¶[°tÀ¾T?œñG"Æš?îi'šM Š?äÁÖ/h?Í7oÓKÎ?~ z?¡sˆ9$l?ˆ3¦šÕåÉ4FGL J0133.0+5931¿ê'Oâb؊ÀP!p"À:Æ(Oªb?À;Ó	¢z@ -Zk[mº@ëùŒHx?Âcwž™¿µ§â1¸ß°?õÄÒG`â?þ-°€0?îIDíoڃ¿êd%¿]"¿êŒ77…¨¿äãÉª¿ÝÖt{'H¿Ä™¢}îÃBUNASNone3FGL J0133.3+5930?Ö¸ªØ'K?Ä-rÐ9.?—;Ëß·9?'ÃŒg†A?ä:™Ì4¹!?č5´¯òR?УT²lòm?Âë¥}Ž¥Ž?˜ä'Ekº?¸;c?ço#ݦûò?»cצ ?ã¯C=+¾?±qúç? fK|,É?ƒì¡8ŠXæ?֞켈"é?°T´‰%ÚÓ?×à"Bíp?³Ñè‰Tãd?»Ä&YÝ®?ˆe‡ñ?ãõ±œ«ºZ?´+©8æ–S4FGL J0137.3-3239?îUowuòÀS§ÃÞ灄À;eEW"&À<Ízí(@']gå@àâ-‡"?ÑB	D¢Ff?ÈÕd.'Ü?ó^"ð•)@sÔ
ƒ¼Ž¿ï‰µ@>3—?ï1g`âC¿é<6a»Ü»¿Ì÷iCŸ/¿ð?ïÿÿ" 5•UNASNone?ïâl™m	Í?-°½1d±?SdÒPw¸?X<Ý2ëÂ?các)Í÷L?!Ʀ`ás?ïyEvÂ^?"ˆ˜‹BS?Vw´ÕNÁ	?tœÛ?'&E?Žß«ãe9?'†"âM?ílóh*?˜=þ²÷À?æÛ«º@¬?'ÔöRuª™?°e'yÐ?"ÑÔø+ð?ï¢&Jó-?tØf³í
µ?a=W…÷?XºÁþ-;?ƒ'a½'
?rrR¡"B4FGL J0138.5+0300?ãÝO=âÀLåùð†nÀ;h¯Á#K_À<¾eò£ +@ "ÆÎ1@^	}?Í[PޔËT?ƒu¤5à?«Þˆ6íg@jÒ/6_¿ïÿÿ" 5•?ïÿþó…õ¿á´ò…Ãù¿¿Ô8ؤ}µ¿êD°~b†ˆ?¶²
>GclUNASNone?ïÞP±%¸ª?lPþZ'Ü?Aޛ@â4?=Ðáâ"À?mn×3w?j_sÎõL?ï·(4?"¯W19?2tÍd"KÞ?HwÓÒÓȞ?¢9Ó_Í?ƒp³Ÿpɽ?î	x_Xs?'á9曾?€Š	9Ðɉ?zԋÜùÒÿ?«Mv+–Fl?øÛàn?ïmǥǾ?w°ßèdT?W+—xž
d?KWÍÜÞä,?ÔQϕç'?v—'—/4FGL J0139.5-2228¿äô~•îOÀSˆtÀœ<âÀ;G-½¨l›À=, ñèH@ÃÞ,ñz¬?øõΞ^$y?Ò ì¹ý?ìÜB 6m@"ÿßHÐ@GYþí¿ïÿtõubƒ?ïöû¿©xµ¿Ë¨qx¾¿ÞÇlüÃ¥¿înX}šŠ…¿ïþœÞGžzUNASNone?܆tìh¢‹?Țõ¨Vø?ßG¼;ÏÑ?ɖr™Ž?°Ç;_1`?®Y'=Âo?೨j\?Òý;Ul?Õ©¸…ÎK?Ñ|'e"Ó?ÁÞ$1Jñg?Àyø±Š6Š?Ò1#ýÞ)?±ÜèŸÃY™?áåí'ÁC?´-Ÿéc†è?ÄAlÿ7'?¤&¨Ý™ü?äšh¤ù´?¹aXËÓ1ú?ÍÍ@ÿyÖ=?¸'Ö|ò?¿'8à$…á?¥ÝžhÁŽ4FGL J0140.3+7054?Ò#Åô㹛@ ÔFQóè›À:ÒIì³"À<k{µƒ@!+µg*†'?ûÑòkyÌ?Ϋæã¤T´?Ç3÷©D\{?ôG÷EF[.@ÄøÂôÝ?æ¹úݬC¿é"³ì+6å¿ãËgÝ^ëH¿Ô§ÿê8î¿ÙÓ¡šÀ`¿áP1ZëßUNASNone?߂o[#çN?ÂC—3Ú?yC÷snÓR?lV±›vnÄ?à@c‡.³?ÂF©Ì³³õ?×P°œ'?Ä!0+"˜ÿ?ŠhMsª'K?•›ùÍr?ã¨?Äÿðê³¾?èu²p3HÍ?¨~®‹owÒ?ËúáÓó?u0œá%r?ÌLv'š?§l=Iù?èCß/0é?¥VQ͛"é?‹/xZ€¶?}ª'gÅC?Í?€K¶³³?¥Øb½~Ž14FGL J0140.5-4730¿Ð77g}ñ%ÀPÞ]öU\À;ÚVùÀ<¦RFñƒ@ªÅZ'§@<Ö!à$˜?Ô4›þxÁ]?Ã6«¸«Ì?è;†ß؝@ðš$W"¿çñ¦¿òÊ¿å…Âýk%=¿ãhN}¼n[¿èãX_<¦¿ïú
!ыù¿ï&Nyà—UNASNone?ï£àï-'y?ƒ*MÆç¥_?On:ÏÜ?Qr&$Òé•?…äö"é?'W!³5€]?ï}J" ¢?'Þ;ƒµ"n?M¿c"ÿ> ?a=ÞføŽº?ŽÑBçãí?¾.-´q?î=£ôÂÅä?)ipø$?€¡ž@ñF?u«çü?§ýY#Ìee?Œ'—>J°æ?ïf¾ãÓ3?|Y( f*3?S´Ñ0_Ç?J"¨â­¡×?'Û¨é?{ÔןX4FGL J0142.5+6650¿äŸ[žûòï@Ö¬¸ZOÀ:Y§uû.àÀ;nŽ	Bžá@¨³0C"ª@,ʦßi?âä"wy3?âHȐýé¥@¶B9`sÞ@z;×F£R¿êÕb{uA¿Ž oPÅ»¿ç†è‡=vƒ¿ël°Í'Åj¿ç#Ÿ!BðÀ¿ïÿ¥œÝùUNASNone?ÓÙh³•	Â?Áò"»1V?ÔRØ^D?ÈñG;^?ØDtS—ú?Çmž•Ø3?ËòN`º‡?´ڶç[?ƝÜù–H?ĉïÆ#¤e?ã[õ)kÌ?ÆcĀ#çz?ÓÄÔ†í?¬WQ7
?ÉV¢¡Ò?®ª7º–?ߐ)(‡Ž?±l%¦¶C;?Îgé…ê´?¯Ë>Iç?ªN)'¡M?¤'Æ"bÌB?æÁ$÷E[>?³'aŽã,4FGL J0144.3+5959¿èw»½¨9À"%B{¦À9Ýv<?AÀ;ŒjýŒˆ@:/&‰+¸@ŒÍ{Hu»?ůŸ)üRÌ?³yéûÜ°?ç@#qPM@J')ÞuÂ?恋ñ:j_¿–ƒaô¼ªì¿çÓ¦¹Ù«¿ëg¾Ö¿èR¬?Ž‹I¿ïúK¹ëUNASNone	?ޔ1ضÇ?ÄWuà-SA?'
ÌãX?}\à{õa?àm¯ãÂ!?Äoï÷1r?Ýãó:ÆWš?ÈöºÛŸäí?xêþ…;3?"J-˜?àÜ0e'^/?Èô·§×1?ۀÛaË?°]Aëø#?±ÏM€U™?"/¨,7ñ?ਫïmç?¯±,©H}?çf‡<Óµ?¨4¯'«ü?¡àÍ{7?ˆ´µ®‡™?ÍþjÙRd¨?§žÏ¬³4FGL J0150.4+4848?䶈µ=À)֊"lXïÀ;•PÔ-êÀ=5²Ñyø@ ÔYM= ?û?ƒ¾f½?Ö19'ò¹?ïöá=@K¡¿	?õ›?¤Á?ïÿFÄ¾¿é9M(¨¿âšýFè?ÎuÎù¢Ãº¿ì
îÛëMÁ¿ðUNASNone3FGL J0149.6+4846?ê™ʐÂ?ÀäS¬¬a?²‹îƒiZ?µ"ª`\ùi?¸«œû¨›?·_ßK!a?ĸˆ™?Ê&¢)UZ¶?àj=ä©K?Ó5Y´0rZ?ÔϬ÷®i?ρÓJ­¸?â­¥™ŽZ?³Ý7-ýã?Ìuǽ`è?°¡TóHˆ?ÈÓ¡ÞTޗ?¨=œ«o?¾ˆ¦§¦zö?¶¯"à_Q?çŽ_¸»Ò?Æ.QµºîÊ?ƒ;-IÓ??»ÑtªY2ö4FGL J0150.9+1230?î`fF¨RfÀGè>ÕÀ;LK?™sÀ<‡ñS"ÒŠ@ZEÚ)ו@U×DõÓV?ˆ#›»_?¡»
²›R?×W"%ĵ§@Ù¡œrg¿âg¨mqó¿ß
º¨²ç¿çÜ7Hkª¿ä›…AÚ¿ÑYƒÅœØ¿ïÿ`h¤
UNASNone?ï¥B͂'Z?~éˍ0=Ÿ?DR¾\ÓfJ?>ÕcžÈ¸?…j ¹'3?}øäÔùw>?ïlœœ¨?Œðánœt'??ýڑžV?VŒ*]Ñe»?Ž¤ê#‹åÉ?‹'I.ì6?îf0«?‰ß¦:S?u¬.-"'i?fVÄêÛ2?«d/›ŒM?Ž×è¼û}?ïSbü`f?~Í"¾;?<E'1Åå?5¸_vÜ?•"Œ9ªu$?~cD Õ4FGL J0153.3+5416?ïþ&•¯ÃìÀ	/+f¶À:êo.Œ†À<‹ú©u°@!"6s?þÌœ†³ä?ċÕ`ÅÂ?"oŒ™šµ?ÐGÖ"¶ä-@íîò;œ8¿â'^⎀¿ãvÍòfºI¿äÊÄ°ž™¿ÛþüôâÀ¿âÉUê`o¿Ïu6
GUNASNone?îS\O $? ñTÚ'?C*tP?>?lëûaT?ª~"\-S¿? Ú2ÝQ?åûîZßê?ų CÆÑÎ?J5õpý?dâ†áEµ?ÓûOˆü?Å£8pÈ?ꡨmÊßÎ?£‹Ž›å?ƒÒG®‹Z?opÖ°S2?ÄG$Y˜?¢F8¢z³V?îsþ@?'™Ñuf?e›LfӒ?YÓC	"÷?§fj‡º:µ?'iaIÈ)4FGL J0154.6+0051¿ïôÜêëà}ÀMÄq´xBÀ;ÆÙ{0øÆÀ<É·sŸ4
@!³uy/A?ß¡ª	SeÙ?è«@UZ¥h?ïäNÿA"?ü}å#çÆ@†?`"¿áýÞ½ç¿ïÿ<h"?ïÒ¯´ì¿æÖÿöÅě?ÎÌc8°¿ïÍ­ÓïUNASNone?넓;2?ÃR÷IêeŽ?… ÚøŠ)(?éÁ¶møW?À"¥d&"9?µ̔·?îï—cª>§?ª4¢ÿ­L)?sq£æ–?'™Ž)Ïé?0ª'h?¥@+֓¾·?êó£ë×J¸?§¯Ð{ò?žvùlÂm-?çZ(C?Àb'#
‡{?¥žð•Çو?ê@€á/šå?º¦Q•èn¥?òÁs¹Â?$+àc]"?ÆûÞ7éeô?º¦hŽúdÍ4FGL J0156.3-2420¿¬THÎó:ÀRÈÁæ¯ÍÀ:ž¯ñʳÀ<ßŠ>²Ã@&âéê??ý²øE ›?À"8#²â–?ºÆÏãÉé?ünà¾Y"@
kRË)¸¿ïþ¬B鉜?ïû .y¿Öôý"U"¿åv" 'E¿Õ‹¥|§¿ÝªßÃ^UNASNone3FGL J0156.5-2423?ïï"Gs¸?b6]¯äÃ?(¶)æbX?";+EòÙ?]ËÛÄã?aÿ7ÅW?ïÙ?1Ÿ$ö?z	Ó65? '°âka0??‡U©—fÂ?rÛÑ©Z*Z?y2CË¡s?îúr4@Ú?ƒé…æ‡4?lNpð¨?g'Ù#\ÆÏ?'ëeþÀÞ?'ÀÎû
Ì?ïÍ¢÷Ïf?aT>ƒÆù™?-ȈÍáF?%ÌË_Û¦?x@·ÏÑݪ?a
Ýt´ '4FGL J0158.4+1230¿îÜÊ^'
ÀG"‹—xW*À:Îû­Šè&À<6Îý(µ+@ÔЯZv@9RKý."?ٔ»#6â?éH#à"å'@øÚ¶š[@O°oó?홽 1xÉ¿çd•ÁGÞf¿ïÿÿ" 5•¿ï5A•Ì…?ïÿÿ>¹ú¿ïÿfb4¨~UNASNone?ïO™'Íü?œý¼i̊&?a1ŠµHÆ?˜MÈkøðÝ?v®¹ACÞÛ?'A'ÚÊ?ì'ĪÂ?ÁFd/Ã8‹?šÖO:\Æ?¯Á§/3Ü?µ4Kdéb?¹û\'l±?èîkE~,–?¨ÌVâk?³(zX÷?œl²ÌÞ?²IbÊ!-?¢!´´¥â?íÇBì)?«gÇ]ê°?g‰Ý*µAË?tÉ5hº'ý?±	™µa­?ªá;³ô¼4FGL J0159.0+3313?éÝF"ÑóAÀ;ÎázûÀ;avؤÀ<¢‡~äâm@ YØ&ÈÙ?ÿ'äÓ?ÇiËu´¸?¶eΐò+?ñÏîTÜÑ'@	Ò¯4‹wî?ïíJÖE¿æ¤œ—zÛh¿Õ°¡]ˆF`¿äÁ—½÷¿À¨W{'ò¿ïÿý¡UûŠUNASNone?ïä y9æ^?j7(Ã?2ò©íõ?XY-ŽA±‡?i(pÛã#?e‡'Ú;FÓ?ïˆóóò?¯vq?FÔÕÖqé?)æ'ý ?ŒbKµát?ˆÛ\Aú€?îVb ?'¹"çè°?hÿÂæБD?hÃ'ÀØ?©	áÑqÍý?'LÔwex2?ï>…ÓÜX?
¾$òõ?E–»W#D?>rèÍpç?—'«'6¸?	Qì›"4FGL J0159.8-2234?çXïéÎÇÀRv¢‡~äâÀ;ªðÏ
•À<ëžÈ­ƒ[@ ö=@RU?ö•ÉæhE?à»E¼Cé?ïÌýߔO®@» 'V†õ@9A‡´¿»¿îâáH2Ÿ?ïÁí@	ÛK¿ÔäçßCr?Î$Œç¯|/¿èÁèm<C}¿Úˆ\ÛMC*UNASNone?îiÞãßy?¢p)¿×›Ø?•ü²@¬¤Ë?"–m¢k{Æ?œàÑâ×l)?›nÿÿª²À?í³mAð?º
zÕ@;?š%-Ü+?²¶mŠ@?§Êö§äó?«æV<ìIÆ?ì§g¦<A?ž•`±®?˜1æt´¾?ˆ}G8{Í?´¸I1Fg?˜Ø7qxÑ1?ìÌŠaÁ?§ñ"{ºôƒ?˜pÝäaë°?™2U ï?µed3Ùx°?¤@x/+I4FGL J0202.4+2943¿ì™b½"À>¨
¿v¢õÀ:æëlËvÀ<Œ<´¼4Ï@ϖ‡å<@áa¡Û‡{?Ä¢J˜)¬ø?xÝmÒ¸c?µ·g	úTÅ?þû€'µÊ}?ëUx™]4¿å#¡Å¸¿àwñsuB¢¿ãÉűO˜Å¿Ø˘"Æ£¾¿Ü­Hãs­LUNASNone?î}ˆ¾ç)?ŸdéÖ?YÁ ò?N)?Ñâqð?§_Mùbà`?ž˜¨@UL?ã›Ã?¥fs>žü?`Ü6Néa?nûþúB 
?¤÷`2ÞáH?¤ÎÉà+\Å?íΘ"¾Vö?'ËZ‰'×A?v›ÒëÒ'?cêÑZG1?°!»P%Ý?Û'":¾M?ì¾òa®T?–ÇóÒó1Ò?uð(/‡ec?f¸èãNÞ?¸°Õéú?—=Â}4FGL J0203.9+8120?ïÏ¥ªÒ"¥@2ݨG²F9À;"Îñj;À<ª<"¸@ §/"R
?üBöõ•C?ÒN{ãüa?ѳôC‰A³?ýT£
[£•@!ٻ̿ëÍÂ6Ƽ?ïÌ$Ñp |¿ã¬Þ²þE¿Ç=:ˆ'
Y¿äôdUêî ¿ïþߤ?åÉUNASNone?ïíÍc¤,V?V}(J=?;½¯a"F"?5º[ÛÝ?]uÌßFBT?Sckó:7?ïœÕBlÇá?‡¨Ø'ïöƒ?N'ŽþµÉ¸?`mõA¨'?†á†tâ«0?…ŠvX˜ñ?îNh2\ÔÃ?Œ›r£þ?€4ùös_?qQ½xŒ?§>'5ô?ˆý§²(ª‡?ï	k©í¾?K–ù´Á?rTU+¦>?cŠ*ðù'}?—©½?ظt?|O>ŒP¼|4FGL J0204.7+6656¿Õ,·¿cG@Tâó¾ýÀ9¶ZöƛZÀ;˜í8}@ݪâ`@ؑüí&	?Á °å¹±?Õ›e Á@°Ì¼Õ,?ý0é5_?é²X­@?‹¿Ö\çÙßZ¿äèÈ%ž¿èÚ'Ér¥9¿ïÂ[ßú¦û¿ïþ¼~K	"UNASNone?­à‹£'ºÚ?¡½'hûno?à~l‰?Æ~Îbcî?ÜïŽÁö"?ÆP'èœã?©Å×mXõì?¨f`éŒr¸?Þ®\~exb?ǽK=Ø?Þè"ïhß?ƊJ\¬?Áøý¶S"?¡FXÃ!ö?ÙêÊ]k:,?´Ú(m?ݶÇ"
?´@øž^B{?¬ˆ¶S%?†ÛFM^\&?àˆÊmàÜÑ?­¼M(äÆ?Û^:
sá°?«w˜¹€ß4FGL J0207.2-1832¿â՚8svÀQ¤Þ*Ã")À;5Ç/ÔÙâÀ<ŒN«^½û@C,[}ª@êB¡e@?ÍSW@Ïh¿wêZ½•ì?§{R[Âsƒ?ónÒHaÔ?êšCb«Eé¿éýöHò¿ßƒ3ü†Î¼¿çŽ"'Ùc´¿ÜÜT^ü噿ïîQ Ü"UNASNone?ïs[u~¾?'ð×ø'Ž"?XPïð8!4?"í-Ën´‰?'Q;æ!?Œ`!è
m?îÿ³¶¥‹??¢bÀ‡ 3?ká]Iɬ?h^}îO?œ]'u¯? Kr©E»?í©Úïƒ	?"lt"®?†—_¢»?|í¨ö3Vš?¯¼w†F?€}jÑ?ì)ÑÕĔ"? O"7GÔ?yt+ –?pwÌވNW?½.—Ñö'? ¹ìbþa4FGL J0209.8+2626?ë"Îa<À@›OKD¢À:묊7&À<P{B–~@ÖMô™=@'°Ì¼Õ?Çe¥`ÍX?¥¥
|P™²?Ûe5ŸŸ@†œñû€¿ßDÙ»J¿å$ #!¿æ› ¢ŒÝI¿â}ŠuV¿æcü^ŠÏÒ¿ï×þŽæ¸0UNASNone?îﳧ=?—® ¬–Ûº?_	Ÿù›>P?.c‰Å? ‡ÎX²C?•¨"¢S?ï.÷óGÜ?–ŠÇmCÛ?L
Îaö™?_äãŸ7?™@™#ôµ?•Ó8ÓÕJz?î:H)ZÎb?ZÔne;?zhñ·?h3 m
Ù?©m,0"á?Š…¦ñ'¢?îÖ_Ã<É?ƒIXyÇ…?i¨~ѳ?V†ŽÒ	?¡¿{ëfX?'Ñaõ;Ä?4FGL J0211.5+6219?ïª<6'
^?ìXu—5À9vZYê
À;?®ª@ÒÆÛD)@ã.`e›e?Æ$nŸDÿ9?¸½èƒažÖ?íêsÁ˜¼$?þ¾¬Ÿ/Ü?Ôh`;©ú:¿àâíP¿é"@U¿å<jŸ01v¿íEO?ƒM¨¿ïï¶Ü gUNASNone?ÕåuÃ(ÎL?…6\ۊ^?›&y녦?"\Ó˜Z?ä4šœ<®?Ã0T"øÒ¼?˦"óã?Ĺ{Ê7³?¥1üÈ4?°]OÛ?çÃ^.ÜßÇ?Æ?	¥ÌÂ÷?Ò[n¨Ñ?¬s!ž'í?¶Ô'éå	¬?˜¨#šÿ@?ã÷ߋ¼
a?¬²m®¥™Æ?ÐûãpQ¼?¨Ë>ÝÂB?º‹ßæWèØ? 'ÚZÄ£9?䣆|Ú?¬_o¾¿õÄ4FGL J0215.0-5330¿Íš|ÖÈרÀM¸H@áqŸÀ;¤†*QbÀ<ër
—@ 
mý´v?@ßËlÂ?ÂF(XcÄK¿À‰¢«'â?ó]]Äuq@ß&–—²¿éS®2­Ò6¿êµ0-Å5)¿áqô¿Zƒ¿×õ·ý‡Õ¢¿Õãm"BJ'¿ïû¥]:ÉUNASNone?ïœ{lò­=?‡Ü‹þ.l?e¬¡-;½ƒ?g§‰¤ò
?ƒuüxÁS?…4Î,¾â®?ïŠSÐÅÑ?')š´µòÉ?A'ºò+'ž?U«>ª1Ú?ŒR\«Òº?l—Êzâ?í̓¨\§?"y4oþÀ?xÐzLИ}?uŽ	'½'Å?°[RYA?"="†5?ï í²
Ô?Œ#ÚÈú—?P•™îrèæ?MX޳߳ˆ?šØðgÛ?Œ|æÙY4FGL J0220.1+1155¿çƒ×&(CýÀF´ê¿üÚ²À;Ñù®­'À<̹kÆøw@#£
VE1
?õS"¬¢ŠÚ?Øléã3¬?Ëv远Ž?ñÌI"®P
?üwŠ*ÍB¿ïSIˆà
ò¿ï웟-WQ?å
ë ¢wd?è7¢cl¶â¿Ç,>¼~K¿Ô''>[…bUNASNone?ï\ê?êð?'4$áJ?F÷z}Ÿ,–?FUîOÛaæ?"ªüHµ¨Ä?'&#ŸØ£œ?ïSù~—v?""•‰m4?IQ'J°?\@×Õ®_ê?"¶GxþïÇ?"@A<DµÙ?í	#vÿçT?œÙèõ¼Ú%?s>~¾äw?fšÜø'z?¶'ü\ ‡?œy6tɉÖ?íQÝNšÄ?§Ï–ýI?=¨ZÊ~¢w?BŒ°Øœµ??·'ȺÀ«>?§Éflj4FGL J0222.7+5016?è%H‡Œ.À#þ½LýÕÀ:âÓº&×ÛÀ<}œ¸2@ –Æ*œ6@˜Ð`Ö­?È\[öu菿Ÿ.'Û+¬¤?Öì˜ú¸B|@L+Dý?ï÷ýÖÚî¿è!"hýð¿â"ëSÏ¿ãÿëþ@bF?'o¦ß…ꙿê7]>ÊkUNASNone?寯üð"?Ƨ¦ÅýsŒ?aH-åæ 7?VåÒ.©?Ô~ªT)·?ƞÑà¿ÿ?çÞù';‡ˆ?ƨ±ÉÓ?R÷S="†?li'€INÃ?Ð/ˆKÖÍ?Ǝ˜¥r?êüú—
?¥°àä?ðã'mëž?nê²
qº?Âí|ù'?¤ç'™³ÅS?îÀ¥ÞöÎç?‹ât7x¸?P<à§Ú—?IÌ¢1©;Ì?£sÁ9Ò°?‹ûÖ5×î4FGL J0224.8+2937¿©Ã–­«õ<À<ÿÜ&Üã›À:¯Úv»œÀ<I½ò>v]@`+ŽÏ@.ȺïT·?DZ%fìÉ?ª;§\6?à‡f%ÎÆ¢@ajþüu?ÀvD?u
ï¿ëŽèe¯‡B¿âsՅ2à¿êcA¹óê¿å•€¸Í¿ðUNASNone?ï+•d€ž?› ÷^_?[ý"N(ƒ?V!¤JfBÛ?˜Íz+Ù¾?›c'ÇØ?îа0–)?¤EÛð¹1?]²/Œ'ÊÅ?p¹f>À¾H?¢kwu_?£"è4T–B?íF§H¢·I?™øªQ£
‹?"uŒÙQÔð?t+2l@G?³<À ?—µÌ"p"¶?îÏ®ÛtQ?'¾µ*[ä?hR¤Ì?Ú?V¾É¶Ãîï?¡çûõö÷?'6 Ýj4FGL J0225.5-5530¿ÚÞ`Å´÷æÀLvi¾	»kÀ:e'Kí>\À;ÑöÌz—v@‡_/es@°yK!?º!ÿ¯"B¿²ìÈío/?÷t'òÜ+@òÎO§Þ¿èï!áQ>6¿èsшô¿â4¿Ÿè"'¿àJ½ÞYÿäÉGNΚ¿ïøHEéïUNASNone?ïý²©?šsEŸåï?€¬V)÷(Ë?í/ƒó¿>?—6HÎs?–àD¼¢Ê[?îôqX%?¥Õ¶ö?h鸌$k°?†¤R'Úü?žT¦jmÈ?¢a[M,Z?ê9sè,{L?ª±Ñ厌´?–3ñðÛ{?"™äKï™?ÄS΁÷b?¨nÌðˆ=Í?æ¹µ&!E:?°yQ
œ·?"¿íd€‰?z`¢Ç_¼?Ñì_´RQ‡?°†OÌÙ÷4FGL J0226.9+7744¿ç€­Óž‰T@/©	¾ºÀ;f6䘛mÀ<´ÍǞ@!Muþ‰Þ;?þJÃ")´?Ð_|½@?º}=msËÕ?ïÎùͶט@N‹•‰¿ë°ûœÄ?ïÐâ (z?èF4AÑ¿åá3÷~Q?¿ØáDŽ$p¿áò,}a¢UNASNone?ï+4ŒEÅ?+^ñQÃY?\0$V'‰œ?'×»³·³"?˜Ö|Iª?–{Ò>bï?î¼¾áQ÷Ý?©¼™ˆÞ3?aTPM4è?ršñS|F"?£Ìæ
3¦?¨{Ú_ ?íž[$ÕQI?"
B….2¹?—o%¡w(?p>~78?±¯æû^F?'b¤E e?í¸yIì?œÚ-ú—Ð?uá¡œ¼?t›B¤ó?°Þ´÷æÚ?›Ÿ‰¥†4FGL J0230.3+1713¿ï)±5±V"ÀCÉ\ú¬ÙèÀ:a"»ë$À<J›ñ@A€§…?š@ðHðŽ?ÈÿQ™Ð¡?șß9¶Úó?ü8­uïpf@QüïÕ:…¿åNµY+¿á†…‰A]¿æ@O±;`¿æAözE@|¿ïÿ"àT¾ô?ê&f%ÎÇUNASNone?ì²åý*Å?²,¶ïO?–/ŠLw?ò?'UŠµkÃ?¹¾†<øÙÙ?°žÓ,Ô ?첎±á¨?µäŠ7ý]?'L^6òd? ˜zú4¸ñ?¶r鼶%?±dqÕGi?é·öú\?§kë6ó?N?¦\ãRð?'CÔ¹Uc?Ù—ÞåÔ?£®謇à?蟯rTPV?®%>ªR­?'%OìŽÖ¼?!}æå[?Ë<˜9ãÓ?­¢…¨¾ì4FGL J0230.4-1140¿ÕNlþ
ÀÀO"[t›À;ãeUÅ.sÀ<åycՒ@"Eñù31?öœªÆÇ©?ݎ½"à¥?ÔÐ&žzT?ù&Ui¾à{@õ•íg¡û¿ï.G P ¿ëÀãàd¯,?ï÷áî-¿ÛW
Ãbó?ʋ)¿A¿â(Ý9+š¸UNASNone?îÕõÿ¦?£aŒò?Wý?[wè?#R?bàŽþã?¡Äè¾~?¢çùìâ°"?ï€iKɌ÷?""x(ÂԀ?NÁa$ð
ì?e|tEü?ù–ûMÁ…?'ä é`?ìá@ªÝW?ÊÎý•Þú?†Ÿå˜ì?téÉÖEÕ?¶Å:5º%?œWÏ
Þ¸?î¸$fÝÅ6?'Yi,†t?

3G¯rÔ?Ô®¡¹?¤vvEQÀº?'X/"-wí4FGL J0231.0+3505?ìAdi¿"ÞÀ7wÂôÀ;¥`úÛ4À<ÓW,6¿°@!õ¸¢žP
?ÝáÓD59?æ¿qdÇ)ö?ïÿ¯Èe_@SÞ|!¹Ž@‰\N4–`?î`pî¤ü¿ì¶´ÝlØ¿êނ׶4Û?䗖ºÖ*¿Ô:睸0¿è'#ᆘ5UNASNone?î"qÄ(]l?¤›€©|"k?ƒIÝ	àôR?"R.×òCÿ?¡öl{ì7?¢ÉL@ÇàQ?îN²ÃTkY?³&íZ6?|Šöžpc4?•b©ç´W.?§ƒtöë>?±Q•p1ƒè?ì_rpC¶? èíŠs?'gu2û?"õÕÚe.F?¸ª99`L?Ÿ8ØDÔ?êëEiäċ?µÄ10r	?bD¾½dçœ?}àõ 	ä?Ä	×]wZ4?µÍ¦Ïs4FGL J0235.3+5650?ÄPw¥¼
À	ŽØ'ãt¯À9­Ž»ð·À;§³Æk‰¼@Š^nJ`v@Ð >cé?Àã[š£~?×êÁªYÛ>@¦Ñµ(k@KªûìŸü¿ÓÌŸóOî¿ÀùÖZÀ¿çA>U¦%¿êœ}ÿà¿ìèÓ=ª/"¿ïÿæÀ
UNASNone3FGL J0235.7+5647?µ$ºÓ©4œ?§ðƒ`¬?ЇÜÕÿA?ÂÓgcâh?åz¢ÙÌ?àǶ5s?ÄDI®»p	?¿W¶*sÙ@?À°{κŸc?¾b&¦î2u?æÂΠ¢|%?Ãáò›×eù?Î×{5e|"?«3¯×«ó?ÔÝÞÕ*Àã?°Ã­ýâï?Û¶c"?°šÂ[5Á?ÖêQ{½Å?¥š'q»Iè?Î*cEÚ?§yÌ&ìÍ?Úw¶ŸO?«ª–S~4FGL J0237.8+5238?êyHL¹°ÕÀ®–ÃüC³À9ÅÛ_6Ç<À<VÁ1Ž…@Vá:B.?üèM&#€8?¾ÎG*`ý?㎧Þ*î@ tNrSÚs@T	|€"¿©q¬]f–¿Î÷çؖڿˮ)7'¿ã®T§!A™¿ïÓ4*…¿ïÛgNnUNASNone3FGL J0238.0+5237?}GÆ!sÍ)?uöÃhïš{?ï"–"
Ì1?"¼ôɈ>?"[J6I†q?¨¿™¾•â?'¹;k€?š>Q<Ïf<?è¿:ð?Ä6öj±4/?ʬËN™'Õ?Ã}~rcÙõ?—­ŽñÑ`¿?'«÷"2m¶?ìÎ rˆ?˜KOojñ?³£›W€‰?"YàšmÐ×?¨¼ô€l¢?‹'Ó£"?ê
µý_1?¨â\86A?Á¥ì†jh?¤9²ÿù»4FGL J0238.1-2621¿ìՏÂ2ó{ÀPŒ¢3œ¿À;쪸¥ÎÀ<°䭔"@"³Ä=1@"Ã9¦?ċšþôg¿Š·t˜O¹ô?Ãþ$@­š@
93Ù?ڋւ®°¿ê3*š}£¿ã›¸øÚqÑ¿ç¼àáVǍ¿ãÁ2d×.¿ìÚ¡oBUNASNone?ïÄ=N~?d"Ü1Á?B7"v ?<M…8Iæ?{šæÝC?~?ò­oŠŸ?ﲸµ:?†´[9ièß?9	_Bh³È?Q¤A
DŠ?'‰­˜ž7F?…yžI¶ž7?î÷"ÍH/?ƒ½}'´Œ]?f—>è8»?U£…êŸd?žH˞yòæ?'±k8'Î*?ïÌS¯È}?aCùõ%?2¬Ì,Šœ?&‡®ksP¾?x«°çXø»?a8oq˜Põ4FGL J0239.1+6634?Ă9ô¡Ð@¦¨¸ñM¶À:!¦+xSÏÀ;¦åßÃI–@K|¯Óí¨@îOá¿£?ËV¢ùê'0?Ì2#(N'Ö@¢]<ñøÖ?ñ
4EHß¿ïþ] o!?ïþ¿Þ§À¤¿çËxÎø¿ã#9 µ—§¿ì¼¦¿Fý@¿ïï–áXuUNASNone?֌A÷Ç\?ÃÈL'÷.?±aø
Ã?¯#=ÿ0Œ?⍠Ð<?Åg=T®:$?À®ÖáÑ¥?¸]V–J?ÍBS*ˆ?ÄìÈL¨Y?äƒèB|é—?Å!lGçô?Ûd_ÿ…SÅ?°&›´˜(¡?½u°"ø}? /©U®6?Ý>3ÛS.?­à¬wü»?ÍÓC°é?§"/<øó?Ðö"R誛?±DՋN®f?àìê…F¹?±ÒJÌí?4FGL J0240.2-0248?ÈùMØ¿¹ÀK1ÿ`Ï‰À:Ïú÷''ýÀ<{q°F"I@ýw:Ê@g&Š®D?¦‡h¿‡¿‡*[?¹ ?Ã@ŸØMœ@òïÌ+<?ãº4¿O`»¿ê{ù?ò^W¿çAÿI ÛB¿ç1‡+ØË߿ҟhûìõâ¿ïþú·ŠñUNASNone3FGL J0240.0-0253?ï|ÆÓ¡X?Ppu(‰–?Y1ö9CPé?QQµ¯¦°ê?Òσï?î?ŒL£ôïø?ï¦N€Þ"`?‡ß‰qÎÐy?8Y ããÈß?P—oaIÛI?…©–ÁXI"?†Íeÿá]Y?î~¼þs?Ò22¸?oc§H¸±p?_Aý韚?¦(9ÉôÇ?ŽMrê¶?ï±÷åB®w?hç!¼/'?:ÝK¾úÍ?1(±É_l?'«Q\'?hn2‡pu4FGL J0245.0+4755¿ì(;þˆÜˆÀ%vbwÄ\¼À;õ5¾À<X;ãv@1ˆc;d@+­Ûoý¿?Ƈ%£¨'.¿˜Q§E1k?ËƟ¡›p´@ˆH®ðn¿ð?ïÿÿ^ðP`¿åMv«Xÿ¿é'öè)J¿Û­"\›Œ¿á2ÚþhÑ%UNASNone3FGL J0244.4+4745?í;€˜pïP?±dz!Àc:?`;´4{?`
™T¤?µ¢œdÜ?±8è·5~"?î(ó!Fµ?·=4šá—K?A'"Í!Á?Zc
¿hÙ?­,Å%``1?·&řDÞB?ëÄT‰¶Šƒ? ³hòÖpì?Á8´ZÏ?{ðv÷ð…?¾%4›À[©?žtª$¾ ?ïÄËQýC?·†œðø?[xïÌ?RXʆùýT?Oטÿ—]?bP¿«4FGL J0246.0-4838?ãåêmFª^ÀM£~õ©eÀ;(×å.ÃbÀ<h¨-±@ç×õÊÇå@µî;²]¶?Äç©Ý^•b¿ºHY`™?òI²Çh	@ˆú:U¿çO¶@ï3¿éG¿å‹<¨&û¿åJæþ§:l¿ïÿýF\I?ïÑ6‰)	UNASNone?ïÒëu2–?vf¯"ú²Ë?f.sӇº?fJ9ºrï?gÉùã#?pÚU)°~?ïDc˜ì?žbX?PÔ®?aÎÃÿ=´?'hú(`p?•Cep¬úÛ?˜©-»cµ%?íäÿî{ËY?"¡#»ÛЛ?€0È!²ÉS?r2*]T¬?­£Ï֘?'h*_=è8?ï
§v†\?‹
¦8·:™?`áâv ?Y1*aíƒ?œ.áb[1?Š;òi84FGL J0251.1-1830?åcy­H«žÀN—ñ{ؾsÀ:öbWãì¤À<pD5¹ö0@!vfóT ?ôç"øoé?Ñ8՟eæ?Ü_õ~F×Ö@Ò¯dÜùk@7µ	Œ›¯?ï0ÒÐòÌ;¿î×Û'Ùc?éätSŽóM?•Q:]³¿Ñƒ˜{au;¿ãáý`"iUNASNone3FGL J0251.1-1829?ë\×Ì2=?º5ä[?£'Þz+î?¡í€…?»]ú'Ø&?µÑÇÌôñä?ïG­Ñ0d?¢t^¨­:?i\¡|Šj%?~Qauù?œKvH¦%? ¦@È.j?讍ÉÔ}?­@ÇÀ+¢?´˜ÎáTÇí?¢ßËèÝ´ê?Âùah§Ç?¥•ë.ëc?émnõ§Ó?µ²R&|,ƒ?lWçIہ?h
œ';Q?ËpDäŒ9F?µÈP/÷Â4FGL J0251.6+0628?Áÿ\þGÀFÉD€bïÀ: ­‹¾åƒÀ<'¤ˆ
%@2au»Ä@ZYÀe¶=?ÄûZiXU?¨«œÀ.rž?á—ÈAíá@ópOžN¿ïn'>´Ï?ì'VÃ[4¿í?Í«Þ¿Ú4çhY…­¿ì_Ïsp:?ѝV}JKUNASNone?ìï>"_©?³pÒ9­N??‰Òƒ{GæZ?†ÓiY¾M?µKºõ™º›?²°N(—¤?ïp ¸3δ?"f¤P-?KœèNB?aā 'ƒÀ?'¹·}?'Èl).?ë¶H1‰d3?¤p+ÛÌÒ*?"'Qœ ÅS?ƒþ1r‰("?½m*Œ­?¢¾"p	]?ï3äê?ýØon[×?n!Ræm0?aAIykòŸ?•Ë™"Õ
‹?€}Äã÷<4FGL J0252.0-3657¿ï!ÁÞÝ£ÀO`˜²é̸À;ŒôNÀ<꬇²çH@ :¬þT?÷ó朁«f?áHÌ!¬"?ÒMÝC¢•?ò+Z;µ¸´@jOøË¿ïüùOâ–c?ïÈNòÄ®¿èEr/ÈD¨?'{o"i©¿æ~râÅB¿ïëá/Z`ŸUNASNone?ïðùiŸ{?\=#
&?*ú~x2ó{?(@ÛQ}[?Z­ÜòÌ«ý?ZÃhG«Ó?ïÌþ©m–?€Á'Go?(Ù#:ÚÔE?DÓv$ɞ®?x¹â/¨Þ'?€08ZV«?î7ýZ
¿6?'yVò~Jó?wA݌?p‰™:Ê-J?©˜h[?'q͟³Ë–?ïªboç¾)?q£¡œ/·?)H¼ÔÖl?/½'±ŸãÓ?…A½ò?q‹ÇaÂә4FGL J0252.3-2707?ï÷72W|OÀO•[0HÀ:Þ\î 0À<¤¯¸k@…kûü4@x¦f0·?ļÚçB¿¨DŸ[f?Û$[)'=@æ"B€¿Ãø*ÞûÎm¿êWådsG¿ëˆ{¯£Ç¿ãýBJþ+¿àvžÝ¦8ä¿ïÿÒkÀUNASNone?ïú‹ßÞÞ?DjJ4'*¿?0Q!¤«Æ?,üæ,wsT?;RÏ\^?Aé'c§?ïÅ'Èΰ±?…É@MQëŽ?30ç ¥ð%?SÓxN ~?|9
H'?"åf{X
?îÀjy´×?•ˆë½?n[VT¦ã?n¿('
Ÿg?¢³¢ÿh?‹àéhùÌ?ïòŽîˆ'?K´ào":?-ìCy¾)‡?(«È¤€H¥?W$›Q·O?HéÓXÄÄl4FGL J0256.2-0408?ÀS¬dÀJ2ýX…ÓÀ;Wy{ ÔÀ<²°9ï@ »Ûۈ?ÿª÷	º?Ó÷e<DÔÆ?¯i³í'Ð?܆p|¿Ä&@GBW=?ïضDË,¿æ
¨ÐnB¿ålKîñ¿Ôè™Fƒ¿ÞZZT	l¿î.R¬,ÄUNASNone?ïÁ"UK³d?t°àð0?0[0îxÝ?$UÛMoà6?~0¤gf9?t]f÷¬À?ï•L .¬?‡¤äD+'2?7­}60¾‡?JTÖòN<¿?‰ïkö'ÎÕ?†ûõxÔhà?îl#ð»Ù?Ÿ+ȪQ?e捆¬?T­_.
Q?§ír"Õ9÷?#¤­¼<¹?ïJ}¯K?{æŽ1N?9x&VbI?1=m"1>ó?–J}…Ž¥?{ãX'Òªž4FGL J0257.8+7044?ܶ–f֛$@$ËYWŠ*'À:6ÄÂ<PÀ;Áœ¸2@»	sq@N`›KJ?Ä̎c…‹p?°ˆ›ÅmÝÔ?ç?	ËZÜÅ@~Ñ{]A?ïï;At"|¿ár%acr@¿æ,æ³'à¿è¬ôŸú†Ä¿çrSÚr§½¿â€fWLíïUNASNone?â˹!?ÇåJ-"?‹]K}™;?€ÛERUÐ?Û~1ÿÂõ?ÈM¨òòz?ä+éâ7°Y?ɽ€¼¿i?–¶2ÅÓ?œ¦zÚ-<ä?Ö<ÊXfÂð?É!P×Ä*T?ä;ۛŠ?±~ia¯¤è?¨±m©_Ib?'ÎQ(Ñǖ?Ôr³š?°9Öє?årv7Û?£y½K»?¥Êèqäj ?‹)ú`¥t?Òa¶ƒ³dö?¢NDq	"½4FGL J0259.0+0552?ÜàvG"ùÏÀFiÕ^kÆ"À9Ìü}"€UÀ;êêÏS)@˜{RÜ8?ýì}6Œ"?º–R<bÜÄ?ÁÔDe_«6@Xî¼
ݪ@	(±‡w@¿ï¶öÁèÃ"?ëX½0w—¿Ý{>ÊÁ¿ØV«ùµä¿ä÷9½ï§¿ì×B4ÍgUNASNone3FGL J0258.9+0552?ïæáÁe–?^–X]]µ?K­Ss¥ù?Fu€!¡?b2齀f\?Yä^à?ïu· ãžç?'u©ûZ¾?KïѦÃ=?bÇ4ë–c?iZžìì?'iÔS7ý?î᠁°nd?‰'Š¶Þ 
?ueƒÉwjå?qC™®ŒÇ?žrŽ×"X³?…ÉMtÜ?îWMÚ´?ŽÌÓ ¸?w÷ˆY"×K?d£µq¼~ø?¬š%‰ã?Î+:Ú™4FGL J0300.0-5908?è2}(ØÀIˆõn¬†À;¶,c5Y~À=™'óe@ 8ÅßÉ?÷Ũ›•\?ãp"'0Fo?ÛÀ?øzDàÑ@hÀà?áÒ¹Ág‰¿çâ,Rƒ[¿âü»§á[¿Ì!ðj¶­&¿àÏà}ƒ¹^¿ïÿ‡4<G¯UNASNone?ïoq*̜y?'/;þ*?mA('Cj?iJî•Ö¶?ŒÓQBÏú?¦ÿQºû?ïF
ٜ?–I«- 
Û?SØï1aØ3?j*°ÄÏV?–Ùg?"üA]&°?퍳*+pÎ?—2jFú?ˆ•,Íå?}Ô
}±ý?°T	
Øs?"|$4ýE?ï·+ۃ?…˜•E
ì?@Ó`'¥À^?DýˆTû#É?œxîGa‡?…}õx¸&4FGL J0300.4+3450?ïԌKt¿èÀ4ìûTŸ"…À:Þ½Ÿ¤vÀ<X®^L¼@pâ²gEß@—XA	µ‹?Ѻˆ¼ývä?Ïg¼&âAÿ?ö	Ã}˜²@…¼:…@?ïæ|Öë3À¿æeÔp/=¿Þ*t]J¿é\#ý`='¿ïÿü¥¬¨?ïH±(UNASNone?ï–ªä,š?"ò¨Šº'?_Æ@}"?]áõāI•?†ƒ~å'a?ƒd²ëÕÚ?í 'ÙÉw?¯@‹ó£ôt?ŒÊANS?–bô€6r]?®ï/Þ_ÓÛ?©,"UÚ?ë"÷á'M?¢çôŸŽ4è?¤ùü>æ‹??'–Jû9€?¹\ä!ƒü?›2RÈ4Ô?êZÓ2Á?¦Æ'«ÆýÔ?œ\*¦m	?Ž>ªÈbEˆ?Äkå"ß?¥¸`#bΉ4FGL J0301.6-5617¿ïà
½PáxÀJZæ[ê¢À;ŒAÀ<ÐRì6 @ 4±âe»F?û˜ç<º›r?ȗ…4²º?ÊU»Gi@½&fœL@ŸØRg?éÏYoØ¿èBã_5o£¿ÑÈ¡jÉM¿ä9[€Ú0
?£¢y^ˆ	¿ïÿÿÊPËUNASNone?ï¹×n.rî?~íÈÒey?SU¢Ð¡¬B?Mü¢@?6?~>à4ž?}aÕõ½‰û?ï墖 œ?ž/üÚ¦sŒ?XCøõRÒÛ?q $	û?šŸæ¿i?›Ÿã·B;{?íÀG3=B?—4	$&Œo?yrÓ=KÎÝ?seA§§š?°f™2A2&?–2
VÏ??î¦ýï?ŒÄ.rË·?Kd®Ƶ?FšØ¼Åìñ?¥1Ð&Aú?Œ™†MÉá4FGL J0302.5+3354?á½ñ×bÀ5…aܓêÀ;!?8$4À<çÈі@!î>tÎ?ýìEz]"?Ë
¯–:|?˜P|Å"‰m?Ðå³£†Œ@9°â‹{?é ð‹C¿ïÔJ«þ?í]@þ"b¿Ý¨áá¿ÝÂ)ÜÓ¿ÔñÌËö
8UNASNone?ïW—7²¤?«­T/?71{£ ¡#?0]	ó´¡F?"°X*}(û?c|Ñiš?ïpí5S¹š?'p\lc?H9NM‰-?^¥©Ôe[€?' Žãƒ^?'©ØþÈ®¤?íŠ2Ká<:?—^ÿ/(¬?e]NÌE\o?S=á«™­?³ƒ*"óL?—(DíHå@?î
©ð³¯ñ?—£w|ÒÛ?U5­t®?Rþ™#?®}G\õJ?—ŽÇ®]Ÿ&4FGL J0302.7+5717¿Åø–$οòÅ
 ÒrÿÀ9¦é#D¨¦À;@«‡ça@'î
_)†@Gá%Ie¥?Æb Â2À?±Ô9}¥Z?çˆÜä.?ýE´ÒÛÇ?îïsàøRâ¿Ø\&$p¿è¾ne8¿é 6Ff—¿ïç"=ç¿ïÿÚÁ,/´UNASNone?ê`œïKàÕ?¼¬Ú$ä]?"(§K>^?ƒ5Ë÷Ž?Å;™¸[ÈÆ?¼AÜ<:\?×A³¦fÉ?ɟ¦\5?5z1
<¸?šÈzšYë/?ãÝz[D1"?Ê0»úyÞ?Úҝ] V'?¯rüjäo?· 7ïݒv?›F"RÍ_?ßeT¦hDÒ?®€Çö£?®?ß*ÂJç¼{?´?V'?³ó¯-.±ž?œÜy£?ÛØQé̗?µÚZ8ðç4FGL J0304.6+6554¿äh=*Ì(@Ü ~$É
À;CY7©ºyÀ<Ç
GžÑ@Üv¸îô?þc\ƪt?Ô|_p#?èç~>tYï@
‹(Øf^@Ê.¸Ð¿ïüÿÐ/WÜ?ïtÿ†]?Û‡!F÷‹¿àÓöAC/¿í«ŽÄS‡¿ïò 
¼%UNASNone?ݛÿºnd?Ĥö{Ô"?Ä%UúLvR?·YÁ«}_?ØQUHk¾s?Æ}ÛÜÂÿ'?̂+''	Þ?ÆU"Ϝ?Ð9uyLvJ?Èâ‡øãr…?àº^µBd?Ëp³ÝÙð?ä ^wÿÿ?°†Jj߄?ÂZ¢Æ©Î?¥&®%Œw?Í#ã\æ~4?©oq× ;?ßEéµhñ7?·í¸s2?ÔÈí2±?¸cí^·oª?ÇâR/˃?¬á»|Iµ4FGL J0308.9-4702?ßEÉWKìÀLDõýG¾ÛÀ<U¾š#À=,jËOõ@"ókò¬?³‰–íï0?ì(ót'Ý?ïÿo¾ÁÇ@FÍ)Á@,xËëÚ¿ïûÁa´¥å?éßð•ÿ±?ï--àôË¿ÚJ
Dý`?Þæ3:¿ïo¿ïÿñò÷UNASNone?î¦Ör£y0?·ó•vO?pÎwÖ0÷'?€OÐ,]'?£xÉÛN?¶™¦P­d?ïn°åHȯ?c PPºÚ?^œ¢_q?†÷òê«Õh?HYŒÀø?—©"à‰i§?ìxb?£€™O)?›Ë'€¾?'ðëšð4•?¸ù[¸ÏÑ?¡ה*¬ˆ?ï=É(˜hœ?'ýʛRÃ>á*ßCA<>÷Œ÷5@ù?˜Dµ'D?'üø8³üŒ4FGL J0309.9-6941¿Ä2¤ÀǹpÀE}Þ?»×²À;S'¢xæÀ<ºôúé?Ê@u~5ºø?øÎrýMž?Ûh«î/ô?îº@ãÉ@Û¼¾aÐ?øì–ց?ï£^>y¸S¿éŒþ–Ž¿ØWæ'öÀ¿éÍΟµ½g¿ï`Ÿ¨žð¿îs´ÈUNASNone?é¨@Pu?Â
ŸiI5å?l£Î‹M÷?nô$Î+òç?ÈìpŠƒþ¶?Áùáo;?ç¹O8¨¸?ËÀâ-Æ?ºgmou?ÂÈøþâï?Ãç"§üá?À"®$Z#?éʵ‡6ød?¦íCó§âú?¯ºpdŠ?–":L|çq?À梇
ûì?¢§=[ 2?âºèDáé?»/y~?³
n"p ó?ª_¡kíÖä?×3ð?»p1—=ØZ4FGL J0311.3+2940?ÝL^Ò73¸À8}E¥ü~À:"å~tz%À<EuU³@Ê®ž8¾@µ¼D¿L²?Ò³A Ùß?â-Ánʸö@	m‰‹.œË@´0©kۿك#€¸¢¿à(ýOK˜¿é3eÞPÞ¿íšÿZc¿ïø`ˆ"?îÜÔ·|ÙoUNASNone?ì€Û§´w'?µO¹{I‹	?´?NM?²ò0o%ö?žè&ø8âŽ?Ÿ@y"/È?ç†ë^ðS?È•;=¾?ÁCÇø{lƒ?Ãm£èøX&?À Š‹ÃG)?¶¶)<fê?å­h¢ì|ý?±™ßÅXl?½:¾ÿxïž?¢´ƒøüKŒ?ʬýô'"9?ªJ⟯?á§jýŽ9ç?µæP«–j	?Åi~Á©ä?¯ó¿vHN?Ñüj¤š)?µô– ¡–4FGL J0312.7+2012?åå¡ÒD¨À?"›«–òÀ:ý=1¹¶pÀ<xŠ§ŽNã@!²ŒÙÔ?û/ä^¹É»?ϞîؐOn?Ä&܍µ
?øI¢@1Hw@o˜Njò?Ûª%?éÌ"C>C¿àMLïœÛm¿¨c¦¬D¿æ¤ ù¿×¾ ºKUNASNone3FGL J0312.7+2011?ïVAÔ6ú?ƒú¹ãŒ´?I4¯~•Þ?DÒ%úsx?ŠW-¿úXR?ƒrJ'à—Ê?ï¤?	¬¼È?†éVÿÄS³?4-æzjxr?Gš§¹ z?†NÎ`ýzW?†J¡GõºÔ?î;§ÈvU?Œ©%|Ôc9?dY×#™ÿš?Rój¿h]?¥¶¨>ú´?‹Â§Ê?XÌ?î×6^yªã?†¸. áø?d8AšàM?WÅ(ñÞ?¡Ië£Ä?†"EFZÊß4FGL J0313.6-7508¿î踱jyNÀCd0 ±»ÏÀ:Äs'ÈÀ<n
Jk^@W)ªs[—@©L_T#n?Èôc>¾¬¤?…sÐ -5Ý?¸ñ›8U1
?úoÒ@):â¿æLœ[ùŒ¿æçeÕFîÒ¿ë"–Þ(i׿ê+ÿ,›i}¿ïÿå"m/®?ïný
Ý8UUNASNone?ïöë7"ž²?Rè⨆"¡?'R"ŠuY ?-Äu끼?N~|ŠçàY?QJ»+˜?îÊësÄ)?°nÁÂ
D?~'—¹á+B?"às¯t"?ª`þQ‡˜
?«><£d·?í¦9"}´ó?"CuzŽ¨?"Ӎœ>ìn?w
'»´;?°3Á¨ŠzÙ?'CŠ[J?ï)¤Zvb·?ŠõxÞtÂF?t ˜£ÁG?n»Z+óf}?•£Nˆp¸Ç?‡ÐŸù}ú4FGL J0314.1+2827?ï$*·8¼À8ºH×à&FÀ:•…ú€d>À<³ûD¯\@éeSi´@_yŸÿh?Ë/¥õrˆ^?À¬°Í'Åj?õ?|Ì@Sp?íf'•ù?ÉYF˜?ÒS¿ìr9}û•¿ÙUkÙ3¿áa?èÅQ¿ïýç¡åBUNASNone?qÒêÅ? ‰ëê¹aJ?ƒ'$ÖX?þ1b'Ö?¡" È)?æmù0¼}?EV$â? —ŠÅSïç?qwÅ,þ1>?HÄuÕ?¢W³ýëµ?ð¸$—?ê©â?ªµvö1º@?˜Ž0ÿŽì<?"Òéâ?Äϕl…²B?¨ÊÏõºô?ìm'|€©/?Ÿâƒ8Ì¿W?'œò¡¼6q?ƒfX?·ï‡s‹¨ç?¤–N‰_4FGL J0314.1+5033?î"dƒÍaÀ—
€Œ'ZÀ:$²øæ0KÀ;È5"_õ@c«¡@¯X}o—h?Íé>]ˆÇ?ÓÒT`ªdÃ@ÉÅ!Ý @¥9Œ=»w?ÔZÙa?ïꧾ d9¿çZ"zy¿äà'÷–¤ó¿ð?ïÿR[§UNASNone	?ædœ´…Ø?Çxù±e2º?¤ˆK|^?£®
ÆDçP?Ð¥½6ÒðÅ?Å×°ó
?â"ú¹í0?ÎÄñ1n‡?™–I´3?¤>܈±«?Ù\¨÷Šºq?Îכ':®?Þ4@ÓG2q?°ª?«|1|?ÂrL0<7o?¡"Bí?ؒ™š±×?­×aÃ
å?êÇ¥în&Ì?¨}à‹1¯P?¤!Þ#0î?"DÉYWÝ­?¿±áŒ}1*?¦'´Q.í¬4FGL J0314.4-4805¿ßúm˜ÀK¡cÃ÷bÀ;NüÕ©À<èŠF?@çÖA•¡'@ ê@{S?ˁ.(\j?¶Â\ÜNõÜ?ë²_~ØÕ@–É—
MF¿êm§¾Šà¿Ç­¹v®³¿äömŸë˜?¿ÜÂ=|¸7¿åÿ‰b"ʨ¿ïÿýF\IUNASNone?ïÌ«(«š0?lHµý¶¼?;-˜"£?2Â"Í2^?w÷›€©±?kP³‹X\Ì?ïh¢/i˜Î? ¡Ò'8?Gtγ­
ð?UCVB
°û?'0/}Û?Žcø¶ËÝ?îRÃ3?‹'ÌÛИ°?xã®e.?jîò.ÑT÷?§ÓRhQ 3?ˆÛ'ÆQî#?ïT
ô?€uu¨Ç+?d%ôOï¼?SɅTRYÿ?šše€pV?ó'ï=4FGL J0318.8+2848?ã$Ê×^À7×UÿæՍÀ;)-c™ÑÀ<¿¹üæp@)Ç`|B@Á#>?Ù	E#¿¹?ïáµA•Ì…@ë¬c ¹I?ÿ'ž=BU»¿ãLYàF&U¿áãùÚLQ¿¯üòü®´*¿éíô?,­¿ïÿ\ è,û¿Ëƒ–¸h¼­UNASNone	?åNÿWœ­?ÃD^©5p?žÄvf§Ñ?¼âüžbÅ?Å>+'!}?½u3†Üû?ۋJöy¥Ù?Ñqd{}[?Úf¢P'Ÿ/?Ò+wöø?Ä%ruñ?º­,³"Í?áÊÀ—%vÉ?³­Ôcrp?͓"ì›­e?±Ë©"?ËAh¶Îww?§®ˆ;Á§ñ?Í*ä7Ht?²S]…¸¿ÿ?â,à+üg‡?¼Öœá¤ÈÛ?Ê!›Åíb?¶å_§½ #4FGL J0327.6+2620¿Û O	—GIÀ8¦°úß.ÏÀ;E'ømd‡À<—ªÉlÆ@!B`E:?üž×¬#ßÙ?áò_£Ô†?»ãâ½úÌå?ãe	ÚtU<@éBb{[?î'ϝ+õ¿èWrþ$]­¿ìJ-J»æ?Óºí¡Ç¿Õ yó$÷¿áâ"I΀+UNASNone?î›ÄÝB_-?£@w£…£?L'PÞëÀ
?\QPêûÍ?¥Ñhè^^2?£*Sà<…Ê?ï:}¹'?™yÚ5&N?SB:*B€P?pê÷báˆ?—|%+wåß?˜lö=~çŠ?í-7F"q?›8lM'g?n›çÀ´Ÿ?bÅö‰oNÚ?µ¦ï®q¼?šÐÒí×?íôaPã‹X?÷ñd?I‡wÔri?R*ÀU#?°)æ‰;zb?è>ç<'€4FGL J0328.4-4736?ï—3÷÷ÚÀJ¢s-õÑÀ:ƒ®E"IÀ<µ÷ڗ«@b±½|ͱ@¨¿§J\?¸ÚÇ6_ãj?"O®ÐËS?Êß«6Os@´Íí^<Ì?Ñ£ø'Äj¿âõmÕÆp'¿ça"oŽ-¿â¿§µ¼¿àá:þϾ¿ïÿþR€ÖTUNASNone?ïêR÷³
¬?a‹äŒ]³ë?9W~:JJ?0üÜÉê?b‰½].|?`h¢ÁÛ?ïÎ@Œ+/"?~-£¾`?#Y¸O½Ò¼?=>°dòrÿ?xDì'êH	?}J·<Y?ï6:ɨ?L£[s?eÈ^uIÛú?W>ñ^_Ȋ?–sLØ叚?|؈HSƒ?ï⺳ÿV?Sð)L÷ÑÀ?C1yxxÉß?3o°|R±ü?hxí¢Âwé?R)ë—4FGL J0328.5+6114¿é0enLls@`'ßBñÀ9¼.±Ä2ÊÀ;wÕ<ÝÖà@¼®'úï@í`Á
ø?ÇV–$D-?ËÕü3Ã@B`Û*±@ÂÅ(=¶Å¿á¥‡
¥Úð¿·<Ê5ñE¿éÈ>O¿çÁ‰¢«'¿íÒEb	àT¿ï©œQ3¤UNASNone3FGL J0332.4+6110?ÇYtò֜?¸"°¼Äƒ¸?»RDɑl½?´ÉO…¨fH?æ¿Z*JÂ?ÀŽ¨É£gO?ؖ·Kø-?ÈFÇ	?¹zL(Ía ?·BÇVÄÌÂ?à…ZÕ×Æ?ÇþáÁ6l?Ö^öðá‰?¯ï\3,=?½qÞ®\?œà}Ž%¬?á"cC1ÍÐ?¯Õ=Ë(¦Ž?ß_ŸÐîRÞ?«ø1'NL?¸'[^k…Í?—Gq~l""?Ú{ÉWvË®?¬MÎ	»j¦4FGL J0328.6-1129¿ï‹]v}µ¸ÀHü«`kz¢À:Òe1³sÀ<"½	á*R@ONœÆ@)ÑÀQ"G?÷:ÿ°Nè?'–¶q2?ϱ^œÃo¬@e-a4l?Ï´UªV€¿è—ñXP¿æ?ªºÔ¿Þ墜!´0¿éÙßÚƋ?ÑZ½:ÞxUNASNone?î'=lo?œő(«?i5^§˜÷h?`"áv'¿?¥[º¯©¤?›Lp;j³ò?ï oêüÚ?–Åé\֖H?Ué‹­G
?c÷0NhÃ{?š"rE%N?•"GA×í?íÙ™¸Å?'	Õ«¯ÌP?xSǎŸì?f8w1#j?¯cír«Â'?É×úI8?íå&Të/s?'î5÷ð?n<nÙJ©Ü?];[¯û™õ?¯ÉÓø^A?'ÌÇ )g4FGL J0330.1+5038¿ç'"ôéBòÀÉHýŸÓÀ:!2m:•þÀ<º«bú@Ó4E@äÀ§$?ÄBصä(?Øü;Ú÷‡á@n¡žJÙB@Ú²šF'¶¿Ù²^ç0¦¿Ö¥›E]à¿ãí¿@r5ý¿ã•#þŒãS¿í«&[´\¿ïµëÿíáoUNASNone?B–2›—Á?~…GðE?Ü(Ëdo×?ń5/Ê?ánY¶?ÅM,DE,¢?¿¾Ó§`­è?·¦Óõž<?¿Š11Ëõ}?º"pž¨‰²?èßdÚk"?Áu1Oè?Ä=l2mã?¢û$³g?/?à¶9³)ƒ?´œféÛ‹?ÕÁÝs‰ö	?°œ––íÀã?Ó9`Î3_Z?¥SõÎÙ§?Ї²æ‰GI?ª4ÿsê?Ü>ìKCY\?©¶p£óqÖ4FGL J0330.7+5845¿áâåy'Dy@-Í9ÚÀ9wb§•À;4ž"ºåD@~B¨œ@a¤_Æ9?ȈªÉlÅü?Ýøk¡Ž°‡@h£?4É@3:·áÙ#¿à6€d¿§ŸÑþ =¿åÔÀdïn¿ï6ci[ä,¿í"äEV¿ïÿç<t%UNASNone?À
ª¦yþ?·ÈK¡ã?Èz5Æ_ ?¿ƒ‰—øc?åÞäù‰˜?ÃëìÞùî?¹ùTûõŽ?À#›ïL?Қ7Í4ç#?ÉF™Â4ŠÎ?ãs¹z
¼?ÊÈË]Xþn?ÆߢŠ[b?¥å¯6Yáœ?ÎIÝÕöb?¬q_rn?âµ gë?°Ž­{ïû?°Š¡€ÿI?Ënf_ïª?ÔAÜùð?¯"ù+B*"?ãÎ%áSXŸ?°£
^xë4FGL J0333.0-3044¿èPQÞçMúÀKRxá"-oÀ;MœÏڞÀ<Ø´*>—ë@FdV@Ô\?ÿ«[˜­
?ÇSÀÜԁÍ?ªhm&ÉîK?äÏ Ä0@©CU,¿í¦M;òõV?ïýR¦–_¿á:ª‹Ydö¿àH?xæò¿ç/jñæaÉ¿Öф!bPWUNASNone?ïë@Îóì?px£;õ[?4üÜ)]ó?mŒEüŒ ?b•‡¼s?]Kè´ßQ;?ïÅ3¹i?€5]hK?(À´bP…[?B¹ÿÖ>ç©?| ¨jl5?LXµFދ?îî†Î	‰?ƒ˜ŠdÁ`Ñ?cß¡d4´Ë?V¹sg¡ù?Ÿ³JÙ¸8-?'ÏqÝö?ïµÅ¢˜(Z?giUƊåñ?Có`¹?1s?6Ô¸˜O@e?OaNaö\?fóËZ
c×4FGL J0333.4-2705¿éªÓ>g*ÀK¶"‹ë[À;=`ðà:À<Øꭈcç@K¼À('?ÿÆü9¡â?Ê}v"q?®†‡™'?äh][Œ@ôôÕ)"¿ïŽÄ¾áQ¿?íôÝ!®¦q¿ç <4cµ¿Ä{ÿÀ?пåÝÞ!ÞÌÿ¿âÆV@~uQUNASNone?ïÒ#|&?jó6¥"ûz?;[é5¤"?2'?ƒV:?uD¯®'€5?iø ¬)¦&?ï°Ãybk?ƒó©D$‰ ?1ïGÞý;Ü?FßêOSÄ?ƒ?§hmS?ƒL¾×I^ä?îUHÿӝè?‹CðeÖbÍ?p[ÖÛ©Â?[®8½¢?¨Ÿõ'Pýž?‰ß¹ûÑ°U?lœ9!?s‹Äîí½?Z-yìE³?MHr"¼†ß?‹
õ›io?ryL¬›Ž4FGL J0336.0+7502?Úö NB@/DêÀ9ŸÏ!:ã+À<Y›0r@\kæ­ô?ütàaÕ.?¹	àÔk§™?ُ/Þ?@ 	ó蚈­@LŽ\¤œ?á%âØo˜¿ß¬übf§¿ÒQþ$ˆ x¿áQ"²ªØ¿í*ÎuCxü¿ïý/k'–GUNASNone3FGL J0336.1+7500?•¼§â—1y?2¬´ØÃ?îÊÌ3[É?œémÍ?éѺÝUt?'¿#WZ›©?¦O‹í	7?ª-6ët?ë­Lx¼Jº?½¸ÉÄêãð?·nô'%—?·¢]	€­?£8'âhBZ?" î}^Éý?ìAZô6f?Ÿ3ÌÑ-¾?´Xßn"+¢?•¯y…!×é?ÃÖD¥5ž?£Ž¼ó)¼?äÊRlq›?°ž4ê?Éqª±(ø?¤•¶]'ç4FGL J0337.5+2423c?Ô;¼9ҎÀ8½ëcÉÀ:¨—,ÊÀ<E»,'X'@#:´†ÚÐ@"WæpâÁ?Ç}–™4?Áo,ž¯N?öŽÞ9ܚ @(Àr×
?ïï"b*—ƒ¿Ù£`rpá¿åSj
_Õ¿æzˆ\Zsê¿áåO_¹£û¿èӎg.UNASNone!?ìŸlÞs?ªÏç>ˆž?xªãA?r"Épþßá?¹'ņ7?©ñkÝ·†?îÓWQ2•º?›wfêÜ?f]ù›Ÿ?tý¾³[ã~?¡d«S&2o?™}n=Ü…?í$ˆ*bKÒ?˜ñ#Ô
D'?…F›–Ÿ6­?rLöÆ?´2ë:ºš?–kuðbBö?íD¢9"²?Œ¥¿ñI²?7»À¬y?j¹üÜŽ?³¿+ö»Äâ?Œ—'δ4FGL J0340.4+5302¿äÐD<'׿ý&^ê–À7½?R%gÀ:ÂÊC…Î@ŽÛö¶U<@Àìœuìì?°¸q`•l
?äéÝ~Ë·ú@*Q)®O3@ÆÂûè™1¿½2t†¿ãˆnßßh¿í³k¢Š¿ï"Ú'—õU¿ïþT~ÝU±¿îmõa™šUNASNone3FGL J0340.4+5302?Ð	󓱀Ê?Ñ«"6h‡i?戋)Á*õ?Ñæ("!ÞK?§'°ÆaJm?°1ݨ)Oâ?…Ú¹	¥b©?œÄJf4£²?ëÄ9~Êto?À?q©~0)?¿"Üèw°1?½û¯Xì?Å´ ›©±Ù?°
¯ù¥?㕹¢-ú?¶7t€÷2?Ëôx۞eê?­	*žå ?ÝïsýÒ¯?
2ÿ'ÑH?ï.+{?ŠâÝ,án?ži\¡)?š?"^'t»4FGL J0341.9+3153c¿ïÿúýóÇtÀ2]`—ÌÀ:4NƒÒÀ;mœzª@/¿@÷C[Ÿc?ԞLœ:Þ£?ÜÏí]æåþ@âyWòÔ@\ò´½âN?å¹ÛÃà•?ÜÙ&wc
ì¿Ù5ä=Àµ¿åÄîs¿ïýà€ˆÑu?ï©ïÝÈóyUNASNone3FGL J0342.3+3148c ?ÐoW%mÔÞ?À±Y-½Êì?¾ÒÅ@J?¸ûo¾f+5?äZ¨‡?ÅUGeø@?èÛ¼ì¡:ø?Æ¡…,,ŽÓ?¹}Nœ'¤?¿ügË["s?¿¤Éþc"2?ºáPb"o?Òò4¤€è?­Ø«M"›ö?ŗsî€ðb?£éˆ"8×?á!²¿t?®ë%¡~Dä?Í¢‹¬sŸ?´i¶£'|?¥G;ÌÑm?—ÙÁ"¿ãþ?çBéc&K?·1Â1õÕú4FGL J0342.4+3125c¿í…)Ü-¤À2©Åæÿ}úÀ:Õ@8ÕÀ;x=õ.æ@N‹Ô4@J·'$1?ç&
{ÅÕ?Á6fC€Þ7?û6jŠ¸UG?î`
­¿&­¿Û›ã`bt¿ãôw JŽ¿éÙȓ'(d¿è«Ë*5]°¿ÐÝg#Д­¿ïóy^æ•KUNASNone ?æݦbÖ+c?ÆB(h{?Ÿoˆ´£¼3?¸ßX=U?ÐMº¯	mu?Ä]×?ý
c?êêZzÌÁ?Ä5AY–A?©CÝ#dé?¶ÀÒµ×?¼=Ÿ—‹?½:ú'EUž?á(Ñ|§Ë?±–*zÖvW?®·åø5Lj?—¢›@¹c?ÙØûžÛ?°Æ²
Ve2?Ñŵ.sU"?¸¯™¥¥ u?€Àø˜Èž?‰êºŽ6ä?æܶdãò?¸äˆ¿Š2 4FGL J0343.3-6303?æ½ì$´rìÀFF	=–c"À:Ÿ–€	¥›À<¬F<$s}@Á²2l¹½@b°~¸lÃ?¿Ù•2+Ì7?©wDã'i­?ë™þ^?Px@¨S¢ivç?îg‡=¡v2¿çÍMZü¥Ø¿ßçÚ$#JÞ¿ä~q f¿Úiœ;_|'¿ãTÝ<†™UNASNone?ï>ÚTïŒ??Ž…ã2$·?djßtd"y?Wyýÿ¶Hb?•—YsóÅ?P݁òKŽ?ï97ß2?'/o?M¸ñæ}
?X#Ï{ÿv?—ë?š0I
?'iºö12
?îê[ÖZ?/§ú'
[?yº²¾ÈVs?j"²*(§…?¬¦ûi?".@8ä?î½Ázpr?"°'ÍGc?sGl'Ö÷?a€lõÚQ†?¡Ã_kf"?ƒÖ£dÛ/¹4FGL J0346.2+3235c¿îÌ`"à^À1?&9O¬æÀ9ç"gnÀ;ˆ®¬Ÿ0@À}ÆC@FÃ1B˜?Ë=+¯†?Êr)H!@Y)Ù‰t@«;[ º ?î/ŠÂ;N`¿Û!ª	SeÙ¿êÜÕÃìS{¿æàáVÈ¿ê3Òê¿ïq"L["fUNASNone0?ä\š˜?ÃtBÿò%?¥ˆ ý)? æ»þ=Œ?Ô0õƒGÙ-?ÂÁ±ßlÒg?뷍¿ûõ?º;|®@ãä?¦°^Bò"?®¬]Îhðt?¶3"p‡‹?±ˆçhÅÎ*?âà|÷WíÕ?±ÎUC‡r?°j<uUXÍ?•?$'°+?Ö$vóúÎ$?¯¡¹"ä-?Þoƒ«hê?¨<º£d5?²>Én:Üt?"á®Nás?ÝWÞ Åßø?¨¸à.4FGL J0347.0-6400¿¤:£E
'ÀEÚà"'À;¼qáÄ«–À=_@©={Œ@?²õ`>Ú@D@¡±?ÔaÝÖ	Œq?ïpaêh@¥€éŸk@óĺÇ`¿ìolÕp«¿Üޝ"µ²¿¸®ƒ5ªø¿äVˀœ¿ì°<]ÔF"¿ïÿÕ"[ʁUNASNone?á
¯‹Kõ?É¥µ+_ï‰?ÔÜÀ>Zjf?ÇØ"a9÷8?ÂÁVW?¸…3k?ÝÇN¹yúÚ?ÏiVùÞ4í?Ô狜,?Ï"δõ‰?Ê¢KTÓ±M?¿Á€$8}?à(‡öu"†?µ¼	óM^Î?Ó3®Ý.Ç?µ"'Ÿÿ'Î?Èö'jïX?¦Å'˜Ù=ñ?Ø^X|×¾?¹Þ±8À$?à8,zÖ?¼#+øû3?½"ܬ0ð?±1DÒÛö4FGL J0347.5+0722¿Ì¯ãGˆ>ÀA"åÞÊmÀ;oH-–;@À<šŒq'êS@!'µ~R?üÃ?ÕØå	?×ÈÛîBé?Ôò–'•¿@µŒ>gCÜ@½l‡'±¿ïþØþ^jD?ïÿñ‡—8–?ÙËëü<üá¿ËЎxSMÛ¿ÌØâ
ü˜¿ïû|b§,UNASNone?߳?‡|UuM1™?\WO Çþ³?WÂë³V|?Š^/ó?†.Óm'¶õ?îõÊûá? 	ùò¯(?\Ɖñ(…?pJ$‹j?ŸzW&­1P?¬ÜË0jý?íGta–o¨?˜Ô֋?ˆ–Êá
?~#2a6ž'?²²ªða?•¯ü"j?íX(Dè'?j†ÙÞô?i
åŽü]?bv/tjü?´vf³Ûå?Hïoç 4FGL J0349.6+4026?Õ¢s	.tTÀ%GMƒAÀ:m@OÁßÀ<òö,A§@fdzÔ@ý¡Ä
†l?Ñ\^¥§ÄÖ?Öf.Þé}@;¹Ïš§@,ý ý{–?ã.žxük ?ïç¶}U[¿åçð¶6¿àH"íˆ.7¿ïÿøÞ£Žæ?ëóæ·YžUNASNone?ã&À‰Ñz/?Äß?³ØéÛ#.é?­ì)oÉÒ`?Ô¼Du"?ç?Âø£Ü¶Pz?ç¨øIÀ1"?ÈÎ2ãԃ{?«£o{é`,?±žBgñ?ÊsBúáª?Æ6Ôç¾v?â ²§€?²Pèg¿\?Áb;Où[?¢G¸èÓã?Ó
"S+?­{áù~èî?èÃ÷kºª?©ÂWÛñ­?¯—þn–?žÃd	+?Å
П5"ô?¥áÔfì€ÿ4FGL J0357.7-6808?è¯î(MbEÀDO
å6PÀ;ÏrÎ\À<öòB9`@!Êy»WÚ]?ú6?Ýe¡E?ÖRÆ«ú?À£ÇšÞ¾?붖à+Ï<@J÷ñé'Ô?àq<þ¹?ïÚÚA)•û¿êòø°€eì?Ì®‰•Àq¿æ۝ }Ç?»ñÿPUNASNone?ﳅ9›Ÿc?|£Ú Áâ?<ó\ÊÌ©…?6¬¸Š?'7²ÁÁÙ?|µ"ì?ï¤îìr!?†AHKÐY?2øŠ#¹o!?GCµ$O2?†,€'Aìm?…';â?íýï1zs?'®ã'Ì/?nŒð¦ ?bÜ[¹x?®F(=çþf?Xö²ˆû{?ï`bXÇd?ƒŠËè³Ðé?V††+ÿŒb?Uw>Аâ?'‹L™Ç¨?ƒ2
;¤Sß4FGL J0358.1+2850¿Äùy~8ìÀ2[YÿOÖØÀ:÷
"ù$À<\ZéZ¢
@°Áü9L@¿­½=Ñ?Õ¤Ùÿj+?ê7H €(.@.Z¡6F
?üÅÈkêó?íÝ	@¢C¿â›EÁ*WB¿â!'o°'¿ïÿýF\I?ïþÞݛ|¿ïÿý{ÁA~UNASNone?ëõ\?¾î{²wªê?´,ÃÜu?¶.üôo2ä?²ÿûüx®?°ÛÈ…?ê6h#'?Ǔ Þ–Ùó?³pa\^*o?ÀZŽ ?ºÜZ"‰A
?¼í¦ƒÀq0?áŒAƒö?²¯e˜¦wØ?Í7GEÃÂ?±4慎¹?̘G´0çf?©·™"‡¬W?æMéh´Zç?Á6F'¿©a?¡oŸPP}O?¨wP 4S—?Ñ69D:…?À?M›[c4FGL J0358.7-7403?è澿)1cÀB£"ý*bªÀ;20:ZnáÀ<ˆ0bžZÉ@e[ç1@ÎàV?̒3ž½ð¼?¦òC~ÚÑr?Øm˵u˜3@fâ(~¤K?št.P}¿•²ù#hæ¿ç,—moo$¿â7¡Â]B¿æb§•¿ïí=±¼PUNASNone?î÷ãŒÛ(?Ÿ}Hxà-?[P•ÊJ?aÀÙ¶ÇÛ;?ŸN…ù»?ŸÐÑ®ZR?ïsë؉Êg?Šóã=pI??leVL$¦?P´¨E¢E?'ÓYm'j?Š¿Â?îþéÒ?ŽÌ'½;–Õ?N,¯Öš7?m…Bæ«6?«VXé揞?‹£_Ù®Ôe?ï:–D˜ãþ?x© pîo?]ôcÜcŸ?K¿Ó¡óüŽ?–Íñ/NÝ?x"vüZ"4FGL J0359.3+3626¿ïá\ü°?À)%òE,YûÀ:…¹ª±À<pÚ]¯@$)*Ü@ú'QT†?ÐtµÍ¬Ç?æÛÊ@«kÔ@êyþɟ?ö¼ß2ªø?ïmíCdٞ¿¹ÄÞýã|¿ç¼æ'æ¿îÛú'½˜¿ïû^°d?îtp–kUNASNone?äö@l…T?Ë(Šoӏå?±%'©®Å?²´ºŽ‰?Ñʍ»D?ÈáQ[ÆÁ?Ümåï?ÓQÎe«h1?Õ«8.´?ҚBƒC%U?ËÏQض‹?Ȇ{–Çt?×ý³Àk´?°×¦Zoò;?Ó
b€S·Õ?±:èÀR×?Ô÷é¿A4w?°ãñ«*5ü?Á€'ßF?¦¢íœ]?×Ý X{_L?½Ì.IÙ3?ßbL"ý¯?¼pp3Š×"4FGL J0403.3+1249¿ì	7ÝDœÆÀ<¬€"ÞÀ:èù@ÉìÀ<'ä™r,@VŒè±.â@?)á{?ÀӚÇA«¿¶ QY9S?ö̯UÀô?ú®ä­³,?ì0©€—j¿ê;÷'X	¿ÞH¿nÀR¿éÐ"¢lQ¿ÑvÒîL#¿Úé<+)UNASNone?ꐑiE·ý?¾{á³qS?€^5Ìùˆ?zý»/Ê?Ä·Öþ‡ó?½ð‡¸Gœ?í*Yì¹'?·®I8'?…#‰\±V¡?–'+™Œœ?´¿n¡î?µ_3堂)?ëUèFD)Ä?¤¢²ì9m?þ'@ޓ?~lðÆ\2T?ÀÈuÂî[?£R/}]ÜY?á©d'Ð
?´gUªwë?"Ê»~Eš?€çCÞ_j?Üásÿ¾?´‡9¦vÆê4FGL J0405.4-6929?íþÍVp¶2ÀC©= ò¾ÏÀ:'3æÊÀ<q´üÌnÙ@*£ÉO•@mt­P0?»‹/ÉqM ¿˜ßÌȉàÙ?ݺÛGŽŠ@	‹QC>™?ëwA 3fµ¿ædaX"¿éË¢«;-¿Û£J<º™¿í°¥)œ±¿ïÿÿ&¦³UNASNone?ïðì½É?^(?$&±?BsJÑíy?CL×t.i?VÄxh?Vò'1Kÿ?ï«-+*X?"ûÛ¨¦[?2y×xøÁQ?Fi?ŠÞvV?" æy¢š?"F´Q¹,?ï[ŠÂÍ?wßäÿ
˜±?jVÂéé?f^X¾»?'S^ÖJi;?s]'+äí?慄Û×õ?jšHÂOÛ?dÚ\09d?TKàÄ"áÅ?€âñýôeÿ?f•´wF¥4FGL J0405.9+3041c¿À‰j.ilMÀ/±_$RÅ À:Å><À<
Bð?˜œ@Þg~ê@%
ÌÜ­?Å["J§îò?‡¾%·l	á?Ãî;ÝPÔ@¬G±"?îß"o–Ñ?ï´÷ù¡A.¿ëqM_¯=¿å8׊•ñ¿áýK 'ß¿ØœbÁì!UNASNone ?ë¢ô–N‰?·b¯¹DŒ?‹1í»«ø?…½ëla?¿'–Sè?¶(h¸‡æ_?îîïMq;? ˆû5Ÿí˜?bUˆxà?n=5?ŸÞó…B¼?ŸÉá"(µ?ê*®b°ä?ªõO¸[z?"¥ð"ÿ$Ø?Ž8v"‹s?ÄÀË3õWÕ?©,Öóïš?ëg
£æq=? €ÿ
>?Y˜(®¡·?ªEOê¯?ÀX–kPf×?žå¡¤Å™*4FGL J0406.2+0639¿ç—oRÂ&À@Ô^'…ÏÀ:£Àd¾À;ÿt²G@{Â4moð@l¬#	"?ÓYùñs¿'ѯà'â?ÐDƒEW@ž0ªlЎ¿ÍÑð£Ä7¿ê1[Xo®¿ëñ±¾SF¿Þ—\R'G¿âŒœÆtÃ÷¿Û|c=gµUNASNone?ìu
 $›?µ6Úztü?v#§žB1Á?mÒI"á¹A?ºõX…ª¸
?´äzº(YS?îâ-¸?¥™"'wt?U¢
Ù{O?e¼Ìæœ1£?¡1>hdÀ¢?¥8O
5¡¶?ê윋‹Ü×?ªÜ‹êij?‹2]é˜Ñ?yj‹æå}?šgó?Ã?©T-Íü?íB=].F7?•ã¼¦œÎ?_K«>Lž?P€ªïÒq?µq«çàÕ?•«Z¨Ü›^4FGL J0407.7-5702¿ç*`og¨ÀF4¯O
"MÀ;/øIRYiÀ<ºª¤ƒØg@'šúlÃ"@Ù{f¨«…?¾/p[áÇ¿¹‹ä$WM?ûúÃ.¾Y@[ŠPÑSÅ?í=™Þ¸Ý'¿åÉ>ÃNŸ¿æ:V=#vþ¿èw²ß:みæ­ Ε?¡>S‰ÈUNASNone?îöçKQ?œ¼>¶ü?m†¦å…?dÁ-D'?Œ"ÁÓÁJ?›À•öÓÍ?îmSõt­‡?§Ë´Û~…?q̹±+Å?‹^ÙL-d?¦úÇ?¤10Oš$M?í¡Ñ½pF¸?"ª¨ó9ýd?ƒÆƒ¯–	ï?sؽyå½ì?°x¡ž‹û?'¤$w—'?îv̳ÈÏö?Ð™T›?yׇÀh!¾?pOšå]?¥XCËeüf?ÐNjf	4FGL J0409.2+2542?íõ½B¯ì±À2à}=B€®À:ÁZˆâ'1À<T3\MÞ°@ x×­{xÇ@#!m8?ƈï-ö?°'ö¸»F?ì2C¬ýú@7;«|Æ?ïï"'`í׿çä‡v¿Ôƒá6]E¿ÓØ-=¥Òã¿æ´Ã { Š¿àPÂFbUNASNone?ï9}Eܟ[?•"J0Gé?Pˆ˜ýgŽ?K¾/u{[?—ÇÍ´šþ!?•y"Ê3¹?ï/bŽ?L?•yÕWê©?Wì°(@þ£?h™Qh¡?˜"ñk´ž?"6´t¤*y?íÉð«ÙÇ?•òç¹Òƒ?u÷Eχª?f|""¢ÂD?²'<°IL?•
÷ š?ì
¯ÝÊÖ?˜n1Ԙøµ?…˜¥:Kb?qCµ(Á?¼ßlp°=?˜Ð~d4FGL J0409.4-3822¿çÚ½/ÐÀG´éNã'âÀ;
Vƶ2WÀ<D@¡±@ ©"- Ê{?ú~e`¬é?Ó듡ÝàÆ?ÜÈ?xæò@*Ï1+7@ŸPW±A׿å P!Öi"¿î؞ý†¨ü¿°‰%BûR¿ÇìÎ_tÞ¿åg쮤"¿å%Ü2›UNASNone?îŠé‹|ì?¥«Økòj°?zq_›ÿ?tä­âmÙ?¤B£äÐ1?¤`ÀÜ[?í¾æ"++/?®gï{jE?ŽÛŽYþ?'Ž
[¿?¯­ßý)¶?ª*~XÆ3?ìE{‡'²Q?£ÖöGßc?'6Xó'ˆÓ?'–Žbò<?¹F††D? Ú>tß?è0w¹ò?©‡o!'í®?ƒEp¯¾g?u¨]«3»»?Î	Ì£îÄT?©EÌ僅4FGL J0409.7+4006c¿Õ¡,Ãàó~À úG²À:'OÐ"À;¦y3Ȅ@ô¾}ÿŠ9@)YE³Æ?Ór½â¤$?滄Üޓ@µŠáoò@02…8cŸ?ïìv`Y‡?¢Â{÷-…¿èòF+]|¿î3¡˜@©¿ïü´%t¿ï¯žŒØÁUNASNone ?ã-Z:W!?ɞ8y\N`?Áñ%ÈÛfÖ?¼NütþX?Ь¸¦ãV?ÆS
<ýny?Ã#Y~Ũ?Ãìº!ÂR?ÖCÅ/È\l?Ï綽¨à?àGjŒà?Îó äè<?Ô5sGëv?¬ðÕðž)?ͪ ?®n©üÑ&=?ÝC7W'ç?®ÚÃD1qÝ?°`2ÊÍÆ?'o1<•)?âØì½~©?·ìmA'Û\?Ö7·t<?¶_0'ÅÕ4FGL J0412.5+6519c¿ê".˜Nú@$c€ÞôÀ:÷e&ËFÀ;ˆ`¾†¸ì@u3Ú¢ù?@±z`ï.?ÕJ*7!?ì~kàùª{@	ÃJ¢»K?ül¶-‡£?ïô´<³¶¿ÑÀa"V¿ìœU•:¿éEV¶ÅúK¿ÞgÜó‹}w¿ðUNASNone ?ÙF¨o¶Sn?Év} aÚ?ÒÕGEÞ¼ç?ˈþ"i³?ÓäJjï«?ÈìütÐæy?ÓHa؍o?ÐhÝ]jã?܀ƒl6Ê#?ÒhÊÂМ?Ð7»<o?Ç÷ĝìŒ?ؐìË|F"?¯(ÔÍ×d?ʙÁø!Û?¯É'a9þ˜?Ú"‰Ó‡¨€?®~]N(?²³pŸªÆ8?¡>p©³?Þé{\··Ã?Åx-ôYýa?Üi¨{]–¯?Ãlñ#·ëC4FGL J0413.1-0304?èÃù]ñÅÀB'žùTëÀ:7]à…ç5À<$'sZj°@‹¾‹–v¤@óæfÑÆ?À·©°=?–"ÆÜüMw?Ò¨~oǎ@8™E5ê?ïê
*%mx¿áçKh´€¿ãåþAcøx¿êkGa=‡ ¿ëQƜ1$¿ïÚúWI'ñUNASNone?íÒ±;‡^{?­=ÜF—/?{§Ü:°?uPÅæKqF?¯_ðÀI¢P?¬ÌwFi"?îëN¢XÊT?˜@‰ÈgÖ?`ÔÕq?m¦˜¥jac? J•m&­?–«™˜p]Z?ì#K['? ßߘZí?š‹©Áš¹ô?‰ÝJïP˜ô?¸DÑ>xH?›¢!K+د?î/5iÒ?‹8N§¹š?‹ÕÿøVRQ?wÙ"ô;?§Œ«MJD?†óB1é64FGL J0413.4-8609¿ÞÃÚ/"À=ˆ]…TÖÀ:ԄÁ›@cÀ<yþ+êi–@U£žU@?ý«>݋a?ԉ¢Á
¡Å?äϺRvÅY@‹ðÜvü@m÷[ÐL?ïüWÔÓ+Œ¿ÉG ½û"Ì¿ÝôÝ5¿è£˜ Õú¿ëJ9ßö¿ïøŸ^›—UNASNone?ì¸·
º?½"š_m?Ÿ'»Ù;{X?»mî×¾A"?·Ã+Cø³Z?°Jòj†ð?ë‡
ˆò'¯?·²áÔF —?žðI'ô¾?¤ËÇ55'?¼™r$ÅZ?²ÐÚeґ?é|¼Ú@×?¨é:"ÿ4?´&m"'›M?š{ÆÓë?¿ó«™n%ú?¡øžPwàª?è`º*' Ì?©lˆ#"ÝR?¤¨ýR?'lR¹l˜?É\×+³½z?§rP˜j4FGL J0414.3+4522?ÝÈ
lÇvÀVn¡žJÙÀ:ð Â'ÆïÀ<4؇3@!I&uà'?ÿëÕ:Y˜?ÈB4‰´t?:9$A†? HŠ]f@'ݳ$A¿ïþ؝»gJ?Ýy¤{õľ?ïßd™¿æÒ®Žd•¿ß^Ù¿¤p7¿äq`Ëò¥UNASNone?èe'_%hð?¿;‰?ZXRdT?R	ÿÕû³Í?Î6±ßY"?¾ò0[?äøYì6\®?ˤ¿Š¤UÅ?QÁ§ëYùY?neã"Yö?ÕýŠ§ì©?ˆ¢7š	?è°2ù±‡?§·f—XØ?'_pk\Ž?y
îìÃÝe?ËGò¶®T?¥´ÀV<äà?ìô¿jjþ¯?¢‡¤™ÑÙÇ?n؀ó\Fl?poÐ¥/f?·c@¥
(R?¢RÛ£ñš·4FGL J0414.6+5711¿ïgà‰©]@͖ hÀ:nìzçý«À<!¬%XC@ á "_Ps?ÿN-E	?ÇoØ‡Àÿ?¹ÝtÉâ?óîZ¼8¨@gք±€?ï¥]S˜.¿Þ#uP5¿ß¥I»ŠÛ¿Ü("Œ,ô¿Ølª'õé&¿êkó™mûUNASNone?Þ²t'…î?Âs#þþf¿?qŽHk‡´?k[°Òà´6?à"¤Ï¬ ú?ÂuCu÷ó?ÝßÍí8?ÅDX"ab˜?ˆ7¡€ÒjD? ¤Ò¨úù?á±"*º?ÅM†Ú®ƒŸ?çoƒs'í?©œ(ãïÈM?'òF#'µÝ?wÒjº¹…?ÐÔ·Ž"È?¨`·U&‡Ö?çc3l"Ÿ5?¦èiEwÙ³?Œqðrñþ¦?{`—,'Ôú?ÐV	£?1 ?§'ōP@¦4FGL J0414.7-4300¿î¸A롓ÀGVìÔªÀ:Ô qúïÀ=Û4nœ–@ÿ
Nãgï@Ü¡Ü^:H?ÆÒv‰Ê?"a(å@I0¾
í)?÷I6W™ƒh¢"K§¿ ¨áž)¿Ýýj#ŠHÄ¿ì"PŸTÄ}¿ïþ‰]aZ
¿îÌhÞæªÄUNASNone?³B]æöÇÝ?µPÐ^uTÎ?ê84á¼?Å<üÞ?¼3àxÂ*=?¿s/Mp?¬ZT!ë7¼?·ßa¸Ô[?ë%‰Kø?Ägï‰Ë×?¸¦®¨b?¹ÒƒËAì°?¿Ð̄+÷?¢Ã5¥@X?æn1dþ±‹?­Ó{ÂUF´?Æ^Ô)Ä£Ú?§ºÄ¹=3È?z‰§J}ž?m—:
kÃG?îÕj'«?–¯±¸úr?žÑœ…ì«5?"ú1ˆד4FGL J0418.4-4342¿éb>Kj6«ÀF¿á2µ^òÀ;ÑÅ6ÖUãÀ<îì$·o@"-¡À»¡?ödc§oE2?áw¿ßÔft?ɼŸV?ë~X€I¼b@¹@œÓ4ñ?äÎô?¿ïÿêÁf½?ïûÞ.ôà¿àòF¿2/¿ï1½è-{c?î2þ…°UNASNone?î"ã4U?·üZ"<?n¤öá¹ö?¡ÐǘH?¤ào'|?µï´þ¹ì?ï8ÙiîÇ?žTqÅrªÊ?]šJ­$«Ï?r}õ/'?œ?@'ï܈?›…p8?B?ì÷¶ 4¡?šB&iû
?bfBð²o?ƒºtĬ?´•þ5üݾ?—ªþß94?ìï—z®"á?¨\×ÙúT?FvÍÆ»É?TvßmŸÚ?¸VVŽÿ5}?¨L
k7øÍ4FGL J0418.9+6636¿ï ZS¹Þ@'¬%XÀ9kÃA2Ð7À<
òPŠ@Q˜âdŽ ?þg:×lc?ºØ6bg©?ظ¤¡µqç@!ŸØ­«ŸV?ûò§b,
?ïÿ`Úá8¿Íù/Lñ ¿Ô9-H7§¿áß¡@,¿íz4y"P\¿ðUNASNone3FGL J0419.1+6636?¢…(Jžæ? ›8èØ?íJ¹œÔ1×?³ÍD'JG?¨Ïd
rC?­Ž*†»?Ž§¾;ß?šæ9¤m³Û?ìچ֪˜?ºÊp?ÖÌJ?µj4Ré‹?¹5 Ð
~?—Ú£oÚ?"^µºð5¤?딪½?£'$MŠú?½šsj;H?¢9—;|?'}îï|¦«?wêÂ9:a?é	"(ú?¬+'5¯t‹?É©õÅnkF?ªÚª:}S4FGL J0423.0-0943¿ïþòÐÜ?ËÀB¨'_ét£À:ûPÍwíwÀ<¿:4¯46@h÷9±?ÿþó…õ?Í\i¢Ûâ"?Þït—'e@ŸÜœM©@ˆë؀µ?è-'	'`?»`̞¿Õº˜b¬¿âuÛ³¿íZ·qõO¿ïùì?®ÁŸUNASNone?â(¹L"ü?Æv}Qymf?ÒgCLd(?á8:v?Ž•ZKÃ?Âõ¤áÅ26?èil '©?Á_H\Œ>?´Ð¯Öm?¶Wo- ëÓ?ÃóvĒ¾Ó?·lƒýžì"?áGôÂ'¸?¸öjëŽ1¢?Ô;§_{àß?·~ˆÛ¹®P?ÂlemÿŸ^?¢œ%	õ8[?羛oØd?¨ZpÔn­?¹WXÉ7×Î? }ÖFYà?ÄYåß²‡?¢Še/oä4FGL J0426.5+5434?ïã®uÉ°¹@ûH
[À8VĘJåÀ;(&Ú@èÛ2k71@"÷Ãñ[ø?­€4¡Oùñ?Ùô/|ÅM}@$ãBؤ@ÿ:)Â?ÉÍ8¤û¿×ÄaÄ@6Q¿çÍù½ÆŸŒ¿í¦Á Hà¿ïü¨'Zà÷¿ì´¿ÍhUNASNone3FGL J0426.7+5437?žÚ¨Èm?Ÿ­ÀëD°?ìçöãÑƾ?³v–»•C?±	žÚ?®ª?®A··L?'#!¨f'?©OM@€ýÝ?ê»ÕÙ´Ñ?ÅlM'²o?Âíœs˜_ð?éÖò«‰±?½t1º¾?¨ëZÆ i?槳¿þå3?´îáé€\?ÆÖvýkÑ?«©#¨¤V?t֌9
[p?`£˜ƒÎùÜ?êíe}€‡¼?¦èaX>/?㵨5Ž1?¦ˆÿ%3
Á4FGL J0427.3+0504?ו5Uf'ÁÀ<ÁR*o?SÀ9hŒs@À;¹ðŠA7@X'ßB@°†£Ð?×9''¦¹?Ã'ǁ&?þ*9ªE¹H@
j»q/ÿÅ
x¹z4¤¿æia#pÈ¿éÆ3k	¿í\¡V&}B¿ïÿ2 ;IW?çZòʍWlUNASNone3FGL J0426.6+0459?ïåÀ¤8Ùw?iJßn7ï?:ŒÉP¢Q?6mÅ ?fí¤Üuœ?hª·Ž‹ª?ï+çî5jT?žxâ£u†?a³ñ‰V?v"Yv¨ÇÎ?˜L"Šª?›³Ù?§Ø?îN£5-Õ?—¬Z…¹?[¤<ÍÎ?x j7UW?ªVþãï7?•UsÛ¢o?ïH=Ãó?RÈ2Ê?fãwi?W¦]$t¨+?"عtjç?€"¿6™åv4FGL J0427.4+6433c?äê×ä@%'"ÂqÿøÀ:.®ZZÀ;¾@=ñŒ@ìýåžÝ@[yJ]?μ~`ƒ"Š?ÓÄ\:é`@nò[Ҏ®@_îZ;4ß?îA²¢i¿…¨ÛD\7¿çžÖà!t¿ïaMl·ä?«Ò¨²FÓ¿ïÿŒ!áÒUNASNone(?ë(^Ó?½ùäXE?°ebٚ?²¼žóÜ&?·¶À£oL?´8裐vD?çÿÂ;ÛþH?ʐðÑDù?§@<é[×?³®nòR¿E?Ê:'U¯é?nj_@ۋ?ájIoÄü[?¯™'U?• ?•¨íÅBŠ?¤ÑqÌn6?Óà˜©"f?ª'꯰Cw?é³8MŸS}?°GÍV Â?•G4wW ?'gÒ3üåC?Ɗ8EÓÇ?®ðøü3U4FGL J0427.9+3632c?ç²sé}À û`'ŸÀ9'É"\h·À;mθ_W@­ÔI@²U'þ?ȾfØ|-x?×pZ›ü@‡è|U»ô@q1¼'?ïÛʖ'¿Ü‹}At>–¿és"ý}™´¿è‰ŠøìæH¿ïèí"Ãq¿ïé¿KÚÉæUNASNone ?Ç%Â	®™?¼HR?* ?´6öÐä1?®»ðÚaXÅ?篰½·Ó?À[æÁVHá?ϱQ=Nw?Æžþþ?ÏE~ËÜó"?ÅêÁ>iV]?àBKýµ<½?ͺ"óp	?Ô@HëH~¬?®Tgh€Ž?Áe
«N? …AŒ¬?ᆙÖ?®ÒV»'b?Ò刺á\E?¤ßH"$?Ðrå…7ø?««ÉT+O?ܧ'¿ç‹Ä?°&fh!Ô4FGL J0433.0+1327?ãùÙ©îÀ+À6©¦
EbáÀ;8×ôH;ÙÀ<튯@ÎpþDéê?ÿÞ5Ìj§?ÓiÎEêœ?ïÿwåëo@Ìã=Qš'@@¤‹¿êÒ2g[Y¿ïénù²Þå?ï½è=–Žw¿×Àó°fe¿ïÌ&´Ÿ¯]¿ïïNÒöUNASNone?äs†Ø<[¯?ƺ/
 {?їJ~ð3?ÄÁÑó¢E®?¶"!a¼?²"×á¥?Þ·õ!dC3?Ñ[oy:8?×ÅJŸŠÂ?ÑU?Þe'<?Ãó'ød?½ñýp%¥?×f*ï*Ï?µ)Ü+Âmz?Üj@¹ˆ{?µm>Œ×æ?É"²7´4?ªâ	ì^KÖ?ÚãFöt#9?Â@éhya?Ú5ƒ7¸?ŋË3Uë^?ÅÎk£§ˆ?´µ¦A˜4FGL J0435.5+3232?²Ù-0a]À$
ƒ{á"À:ºÁ濽À<P[¡çEõ@.v‡›À:?þÑטةz?̍ø%ÁÃ?ØèÒý='í@	ñ9þÿO@õõ•måâ?ìÀäbÈ?íúVrÓ\3¿'Š FJÖؿމlLþ¿êz:Ä!, ¿ï"ž"?pUNASNone?ÐÒËåt
u?Á8rKLd»?ÂGô,œ/?¶l÷!Á8€?ãِ:Ó¹?òÚb¸jÅ?Üb¿GÑ.v?Ì312š?´¢U…Üœ'?¶gëÝ5?Þt«V·ªi?ÌO²*÷M%?ä!7ñ¤j?°>¥ß/?¿Œ0yŸbÃ?¢Îq݀o?ϵþÁ¼õ?¨áZ÷Í?â03uékÕ?±Ál
?Ŝo}yá?­îå+íù?ÐÑaUpœe?¬°+¡è•4FGL J0436.9+2915?ԖY@Á™ÆÀ'äAVâdåÀ9ÐϟåãõÀ;wˆ4íG—@3·EQö@Œ²`9ü{?ÁçZS<=?ÎbZû¤&@ú¹o!÷?ðŒ+$U?Öº'#'à¿à·n=h¿ã|¨Ý"U¿áüî
ö¿îLb-<¤¿Ø1Æáü3îUNASNone?À‰ÿ°üÞ?·]ƒç˜˜ª?ϛ•›r­?ÁiΫ,Ñ?ãöš¬äU^?Æ
HÛÄæ?ØÌÛd[+?Ð8›Ö³H?Ó7ª*WŸ?͸xqUú?ÓûzÀDÁ?É«HKav?×öy?±,óÛ
!6?ÄW LñM?¦"FÒÛ?Þ´y`pfÉ?°1òóJÝ?µ>yÔ=WÕ?"êø$kŸG?Î
m6öª?®æ+?b?åՕj—[?±Hì!¡M4FGL J0438.0-7329¿ïŸ
Vg$ÀA—ŠC»@³À:n¢‰,dÀ<}ƒêXÏ@ ¦'æQ?üADˆÆ¿?ÁÅøâG]?´P°Çˆ•:?ó°¹÷2ú@¤h$V¡w¿Ü½ò%Kê¿ìI‰¡Sø%?¢GŸë‡¿ÙàP7Oøf¿ß\*Ãx[¿ßd3›¸Ø¤UNASNone3FGL J0437.7-7330?ïuêë}>?"¼1ï*ÎÚ?GŽg­û¯?;õDnA¿?†/a zª?"VS®ç½?îþ¾sº}?Ÿ3ÐÜäDr?P'iÊGp,?^nZŒs‡?Ÿ
ìåü?ž"ä`Èc?íß׏\FÕ?'6çý&5V?sEù֊/\?a=¬õ0äÚ?¯™ÇÏjL®?dŸa–?í§
ÅG¨Õ?'t5t×u?g¹ÀµEI?WëNN	4?²	Ûп(?'0ì.¢ÿU4FGL J0438.2-4243¿ä#äß>ÀDø¿p]À:¾Ú`3FÀ<Lð\@D&äpX@g ã¥Vf?Á"žy_g¿®	§ô{<Œ?í®"áÉ´@¸"ŒòÂ*?äYo<νh¿ê$DîFš¿æM™{f¨¬¿ê—v©ªˆÕ?γŠ›úÇÝ¿ïÿæ4|ßOUNASNone?î¾R¬›Yd?£t'¼2?vìQƒø?uØ=š³?¡YRxÀ95?¢TT•ó+?îÊ0^ä°?¨N:Ì©É?c±	(2ªz?€pFÝ¶?¢!郞ŠR?¥îH¸ºg;?íDˆIa´b?—ñ6=|ÜÈ?"°CvG\?vÑŽ:?³EµQc"ÿ?–.'k)…?î"Ço·‰?'êpòóÅÑ?P¹y[f?P"F
MI?¦/B;"œ?'½Ã»9pD4FGL J0439.6-8322?Ù²ó¥Ý'lÀ>•Ëeè'À;%Y>_· À<€RnM@"wïвà@ˆ:Ùð¡¾?Ó?Õ"[ʁ?ÇĕEÌé?ñ(º3m?üNøñ˜ß
?ï÷¿¾€^då¿ãY8œ(À¿âV•Ù¸é¿ï]]ÿ¾¿Ù>Ÿ¿ÎbUNASNone?íîá[áiê?¤ÏßKäM?z"FRU•d?v*"1jb?­Áawž®­?£ÝÖ%Ê)?í½°Ž7]ñ?ªr¶§?ÊÏ\	w?‰ÑÕú‹?°Θ"w…?§Rcµ4à?ìϟãÿH?šK"ø?˜oS¢Œ¸ú?‡ÕQ;Ÿ,?³g+þ\׃?"Ü'o¡T•?ꝎŒNN¼?=ŒNTÇ?›@Ác'J0?‰óú¯
²g?Â!­¢T{É?›÷\OÓ«»4FGL J0442.0-5432?áG5Ò'ˆÀD/§íåÀ:¸8!ïÀ<¨»5˓è@/ëï|Ð
@g­"ãY×?¼ï"ãñ¿­ëþì.¼×?ð:µ´)@v•]ŸÃT?åsú~
òͿ唐æl±¿çÝB 8š¿ç¶Šþøï¿ïÿpޏlð?ïýÕM¤ÎUNASNone?ïÁ
±ž?{·OxBZ}?dúíåÝ
Z?`¤ƒ–èG.?tû°'¬!?wJy¬Zû?îù³¯79w?š1lÉ?`2•>¦ñò?oGð©Î"?žÃ7qCòº?˜8DüV€>?îAÔ¦.Ú?'
0RÜޒ?'ñ­ò?w†—iØý?©nñÍÙ?j0tð~µ?ïn¬Åz¿ñ?yÊó)ð3?u.ôɕ:L?h6ÕÃbV+?‰½T<…fÕ?t·$–$4FGL J0442.8+3609¿ïÔ{uþE&À¤¡4˜ŽÀ9×äQMÐmÀ;ƒÔA5Tv@QBŸ@f1rhÓ(?ÆjEî÷š?Ño§BN¯@*F"bH@ªÆ>¾,¿ÉEø\Ȃæ¿ãß¤¬ó¿è€fAÓ_
¿í¤]­Z@¾¿çIžÚv.¿ïì‡b_p©UNASNone?Ô"<k(?Ä7jèP·á?£+=ZM'Á?¦#Ζël?ä¼L<ñP?ÄËɳì$?ÑFØdõI9?Æ	@8ê?¤äRû$v?§iÇۖ0?æRØU©?ÆÊÌ@VÆ?×åR
˜?°D
Цº®?½Iï¢ýAç?œÛ†šü?àdÅK÷?¯s'	ɍ?Õx0cÅ*{?¬
~tÉ?·ÝÛ%Ö:Ý?ŸÝtŽ l?âH,ib£g?®"]µr2¨4FGL J0444.8-3514?Ô ×œÅ¯2ÀDçÝÊKÀ;k%ÈçdÿÀ<Ëå+hc—@sÆxIè¬@®'r—Í?Ð!DÚ$¤?°g3BE?Ü´_c@ý'öÛ?ïÞ43
s†¿ÙæFñV¿å"ÈA!ÞL¿ïýàÀõ~?ïàŸ°4¿ïñ$ЙàçUNASNone?ïÐ6L®LÜ?uP+hðä?5xY«3Ô?5lu7õ?vT&Yô?t¸\¶ö>?ï/ý›MLX?¡O¢tʵv?^ßß3§\.?{'ì{ãàÕ?˜N£ÿ+?ž6ühn?íwŒßÉH?"}ºëùo–?†7²Ó]ª?yxH³SP½?±|¶QJ?'8V,Hw?ïÍqRb= ?qUÓÀ[ñ?]FÞh–?aS˜Í¼J?yá³i*]?q;W€04FGL J0445.7+1535?à[µ2|TÀ2ìUC(s½À:FE­‰:§À;·áñ÷ÿ€@ĆØ!@Yx"væ?Ó0p ¦ÿ?ÜBéŸ"w@	˅¤ð@ÐrùòŸÅ?Ѭ9d$­¿áËF¿Ä§¿èO¬½ã¿ï~µè"¹¿ïºú<q V¿è…™!y¢XUNASNone?é¶è›ÎF?Á—½ô¯?¨ÃBÏ%¹2?¤ª¬ÚÔ[?ÂóÇXž?¾ŽcštÒ?èfJŠøBD?Ãì®ðÈl?¾$íW¦"<?¾Í3ÑA{?¾¨¾P—Ë¥?µ,Ãز0³?áÈ©@
ž?°"=×A	?¿û^Àð"Ý?Ÿœþ¡÷´å?ÔqýCÅÍ?­È‡BÂçî?ÚŽ_ñî?¨˜†x¢?¾´®É·?¢Î»	Ÿ+?Þ<k£4[¤?«ùµœ­T44FGL J0447.2+2446?ïÿ:¨ûêÐÀ*]ÌcñAÀ:–8¦ÿ´À<LB‡ö@vWNñTÁ@æYeÌãs?Ò‹eNce?îÕëY€@~¿ù³?üµíbC—?ÙqÒàãG?ïÂQHÇïî¿ÐÕao0º¿êÕTáä·¿ïÿw¯d:?ïñ™À…ì"UNASNone?ÈN<ª¿h?ĊM;IGÄ?å3mZ\?Êeîô‹ù]?Âåi ‡Ðs?ÁЂÑ+?Å)MmÂÌ?Ç÷xU"i?çV|8-Ò¸?ÌjÒ¢tÅ?ºøý£µäª?¹…¸óÍGþ?Çnbq؎?¨§lˁ?âŒMÇ@¹Ù?²ÊëÄ
ø,?Î`9€‹@?¬ÌØÆòw}?ªÚłž˜é?—"uAœÀ?êbX]æW?±^
­ubX?¿'r{Á€Ó?«à¾"ÌÙõ4FGL J0448.3+2743¿ãÌ[°!À&TŸ"…^À:³jû÷]À;«Lg·Ÿ>@]EÌ=î@U8áÈÝT?Ï'öüK@?ҝû¾|Òä@*à~Zy@¿"Ë(²Ò?î–éP'¿Â"ž'¨'¿æ[™ï)îç¿êB­#º¿ìùYó'\´¿ïõø	'y:UNASNone?Îc0ðÖwp?ÁO{.ÄR?¡Ž–çØD?šÞ"Â-_È?çOÚ[ä ?Â[êY¡S?à¬o}­'?ËSKyêë?±å)ã?°kŜò=Û?Úb謋Þ?Ë[ý¢½¹™?ÚRìS†ƒ?°êûÅeÁ?Á'ãì‰
?Ÿ	Ä1>
{?Ýh»gôy?° H
*:'?Ý2Ì'¬1?¨|§tÙáY?¼"uM"f?Æœ¯F@)?ÛĖ"îÞ4?©Ü
`r_4FGL J0448.7-2116?êÓ»aÌúÀB€ýÁaÀ:wSeØ¡íÀ<láçDò@^¢›öÁ@‹Âßä?Å,ËåòÍ?Áǎ^ýçL?÷ÈÙm²‹@Y>:"e±?ï¢1þªÀ]¿â«¼|±¿è¢R_ô1k¿ãinX£/E¿ï½vþ«¿ïð­aÍzrUNASNone3FGL J0447.8-2119?ïßMÞÅō?fÂ8‡ê?PU{³m`¾?PñŽ‹í?h‡c`ƒÂ†?bLo8éà:?ïh½ã??ˆÁ½ç"áú?=67x/YX?U3*Û?‡¼Gŵ?‡.«±G§†?ï2`H¬qH?~‰="''Û?jÐ%ê'ÞZ?[œ>|+ß?–Yò-,Û:?{Ý+ÕAü?ï¬1¥¸Ê?g'>4ðãÐ?a0ÚYOpß?MÁéur¾g?€§_û¨1Y?d­-O¸¨4FGL J0453.3+2843¿åd_®™äÀ#
çöô¾ƒÀ:3á @è(À;¿p¨È@ÅXQzÆñ@%ن³U?ÈVãçp'?Ñ®äïÙAO@»Ò#Mââ@ðßP²ö¿Ñ=˜|c'î¿à£'÷Ó¿ämä£P¿éæg"N¢¿è4©TøÙ¿ïøT<jUNASNone?æ·®ƒ¢Ê ?®«;	?'4+Ÿ¡?{" ©[1:?Ò¡W]m¸?Ât°àYÍ
?åíR ßã9?Êx$·í«?"\KÌ?'n÷ÿ"¥¿?ӅÞ/g0?ɜÇo2÷-?çÚ(ÁPºj?­§Î^ïßv?¦'ý°?)Ð/[œz?ÊöÚûQw?©–5o&£?è ðpUšø?¤ú<£?‰.n
œþ¶?s"=Ê©¬?ËéW]ÿÄ6?¤|ñæA¢Ó4FGL J0455.9+6757¿º¦»¿o}@.NޗÐk¾À:ô§vÑîuÀ<·ö:"`L@ ‡y{ Ô?ù¦,ƒì‰?Ó#½¿"©@?à¸æÁ?¥Ý@€':O‡'?÷ۑنĀ?ïè;B¡:M¿íÊJ µ'-?³Ó6sXg¿ÓÏF0Š¿éBas7…¿ß?|žJ®UNASNone?éL¿Œq	‡?ÁØTË^?°Ô"0Ñò?—ÔïՄÛ?Çç;µ¿¢?Á`ï±<[?âӑ͆gÅ?ÎZ¶]f£õ?Â?õn­õ?—¦1ÿnu?Ñ8áß;Ù}?ÈÄXž!?êfã·ÂV?¦¿uÁ6³?¤?Jké?'€0	pL?Ába\¤º?£A쏸®Q?àw®ûí«=?®kep•?Áb´z½?©»ßE`«ë?Ö_GËJÅ?­ý€*kÁ4FGL J0459.7-5413¿Ïn+
Â,ØÀBíZ[–(ÌÀ;Vµ–Ob>À<è،ôo©@û¾Ù6?þˆw'î\j?ÛCú*Óé!?¯9X';§ ?Ðú`ƒÎV?ùêmÿâÎÂ?ídÈÁû7™¿î;.¿±q¿™]©&¾8¿ËéÙøÚG¿á#[NÛ/f¿ïÿ%ålÖÃUNASNone?ïŽGç?'Þ`ž'È`?5L†¤ 8}?2~•£Ã:?‹Ïy"K?'Ë
L}ž?ï 05Í?•Þ
@D~~?P} "ÍÍ?^S_S‹?šò,v‰?•¼ûH›?íû2ÂÙ?Œ%Ú?ruxÃР?cè&hD…³?­þ!ÃUÄ¢?*#éª?î·pI‡Ó¸?‹®Zë)RÜ?VþŠ³nmd?Ré
å|^‰?£ÑçQ?‹iтӝ½4FGL J0500.9-6945e¿ÅšH~|RÀAeÕQ֌À8¨7æ÷~À;v8è†@~ÕØd/ª@Óo1?¦+±^²<ÿ?REbåÇRa?³WÔþ©c@=`4H1?ïçë ÊÐÉ¿Þ[]‰H¾¿ã»üР–ä¿àô÷Ãñ[ø¿áF]v'Ï¿àïኟUNASNone3FGL J0456.2-6924LMC-FarWest?êåÖ6Vº‰?»{–‡_?q'Qœkj?jÚe'¾¶;?ÃßnL2?»üKd°ç?ïóqûÍ?›2ñ¬R±È?Zù'ÚB ?mç¯E_F2?›ù®\\w?™s»Ê­_ª?ã$½ƒ« ½?´7ðÔ$™?¢þã'ßS/?·N<&
?×V¨†mÔ?³JòB<ÑO?ì	Øz¨/?¤±mÂð)E?Œ^"^Þ?wIµüpŸš?¼%}ÿÞâÇ?£"ŸfÃ1†4FGL J0502.2+3016¿ærý7½uÀ+
€òçÀ;)ÿ­Ê©À<7b• Ž@ Æì)Œì?ùِʽþÔ?Ù¢‰bñO?Úìåq?ûmªx.—@,XÛäAÞ?ïÿùëñ¿ïýÅB"Ð?ï}[À›<¿Öèf»ö»´¿Ô©n)©¿ïý'€›pßUNASNone?áö°Î',ÿ?ÉÓ5O×d.?wYÁ/'9,?uÎ~ýº3?Ûµ7^õ	?ÉÄß½ÐZ?ܾŸÔ!s?ÈwUrØ?rc)ˋ4?ˆxB¯‰¡?á{êüX/?È)®ð%o‹?æI2Ÿõ¬?­¨‰žbþ?¡'s|¿?Œœ…_|©I?Ñ;Vÿg…?ªØÞà
:?çÕ¥h/­?¶Ø\%Ó'?_ðÍõÑ[?^BêircT?Ð4Äû:ŠÓ?¶ãy–ÜØC4FGL J0503.8-7508¿Ôò8ržiHÀ@ztBÇû­À;U­…ߨrÀ<¤¬Okx@ÆWÄb&@z…ص?ԏ&#*Q?Ï1¾{{?ñ'ºÄŒŒk@_[]ˆ¿ïù "_Ì?ïúŒž3‡A¿ãb°Ï@E¿å¡"ßþع¿å"PŸTÄ}¿ÚEÙ]ÔÇmUNASNone?ïFÈP²?"q"WK«Y?d•Ít",?["Ž3Ÿ9l?œ
íGe}?'ÍÙ[æÚÇ?î€LVKb?¤TôPÁÉ?hиÞ1¨?v덎܂}?¦n/Ø9s?£
ø}áÿ?ìäŸPôÖò?œÚVÛ+?—Xúãpî?ˆA€ž¶¦¿?³9 l9?•o|šç
?îS¥8ÝX?‹ùzŸü´Š?wNbÁ]íZ?hä;0C?« ùTFlã?‹A¥È:È4FGL J0506.3-0620c?âWŸ¨k2mÀ:6ŠçO/À:¦IÚ>¥WÀ<O%üéË
@©{%2h@š±ý=­à?ËnŸšåt?¸d ,?éžu "se@JÖßuEý¿åEv+ÖG ¿æ0©€—j¿âhx>Õþ¥¿æTÑ]Ö¿ë®IW¿ïûÍÖ¸UNASNone ?íƃ«‹¢?®iÖ¼UéI?w‹k²ë'?n»¦Ð§?¶`+ètB?­Éÿ"\'ò?ï
I,x?•€¾2·?ZÙ¥a_Ój?j1û¼]'«?	@ÙßC?"u£X̝è?í=vú–ç‡?˜PÕ`™?Ézz?'Bîdªî=?±âäª%??"$*2Uo{?îdèÑ?ªC~]m?v+ÚÌ!õ¤?c¯«m"…®?¬´6&J´=?ŽqÝ5"4FGL J0506.6-4629?â6¿Ú¡ÀB{<`ŸÀ;v?""ÆÀ<Ó§<ð@!>÷þSØo?ù(¢› ÚÖ?ÒQ>a¸«?ËkÄIE™<?þ5ctCž»@-œsÇ-¿îm"wú¡?蔩ÀXJD?ïHã—­¿Ý ~Dÿcx¿ÐYGŸœ¾¿ç"…U>÷UNASNone?ïoœ¿hñ'?‰xq™¹l?U}"«óÍÚ?Pn8Þã¢æ?´ŽÈ"žW?ˆoR_Ý?ïw¦Kbª?"¾MvQ¦"?A1|¢hz;?XR¬MèkÌ?~Q€fþ?"ˆ8¢	œ?íà#‹?'2vƒi'Ô?uHT,ÁÇK?dÁ0æA?¯U3IUþb?'VU•eß?ïC^Œi!;?"	šô"?EטÞ)êÿ?E—b$٘?–åq«ê‰B?ƒâ²žÊˆ4FGL J0506.6+4545¿£5çŸ_L@

Ý8TÛÀ;@{¶YÃÁÀ<r%ÿn	É@"‰ioZUâ?ûŽnD—à?Ö§;®+÷Ö?Õ¥±ÀVò«?òésçXiN@ïÑ—Êâ¿ïÐaò¹F?íÈúz…\¿ð?ïÿþBe«+¿Ó`dYEìs¿ïþpéw'UNASNone?èHN°ýÌ?Ä%3²é?yb^ÝBP?w-ÚOõj?γÎQø?Ät(I.?æö'»O¤?ÎåáøN‹?ˆÙÄa?§í"¦ž?ÑLþyÃ?î?Í©ÊÂ-1?è\z·ÙL±?ªgüUÕÿ?š üÑ^?…m­
ìÆ?Ë>!¡{?¨tqxàv?ì1шlÙ?°0"ߙ_?¶/0ø?š–œið?·h宸Ìü?­PÌ3é4FGL J0512.3+3329¿ëÚaÔõÿæÀLF__áèÀ:v9´V´BÀ;üz,€@ ŠŸb0?ú–=Ć­.?Ó¥àú¬.?ÜÖÈäŠÙ@æÎãþAº@0@0Fĵ¿áÒ)˜¾&¿ð?ð¿Þ¨'¤W¸¤¿å>8ŸÙ¤¢¿ïúúý·¦JUNASNone?Û©À̔°?ËU¤mV+?‰CSUyd?…Û®Ì$´Î?âÓx_Ã?Ë|¯%A`R?ÝÁ€ûâá?ÉSÂ
$Í?r‹!.fW?"¾:/7ҕ?áNœ)?±Â?ɼƒ*?âV>Òb!?°õÏïðÙ?·¹õ¬/¾?Ÿ+ÊA_?ÕeðÓsÐ?¬Ï‡7À"?åd5hÀtD?¹Kfe`LK?{D=yúDˆ?vµ…è`±?Ôʄ8—.f?¹…,º­4FGL J0512.5-2201¿ìíüÕ¤À?êÈ`V'À;&k&¿‡jÀ<~ž43
@‡k;p|@R ÿT–?Àv_'Çp¿¾,8Ã
@³"ý*bª?ú–ÆXêR?ï÷%  ¿åø'Už˜¿ëÝLâ0â ¿ÞµíãðQ¿ìn<ô}ÿ?é¢ áÌäUNASNone?ì±e‹qd?·'Ô*~ú?ËE'"?~"MÆŠ[?¸RÝãČ?·#¡¬ԍ?ìž)ìNÏ?»™èžm 7?'ŸWð~fœ?¤£n¾{·ã?¶fÚ£Íïç?¶ êµéÙ?ìóºžÐ¿ø?šõ¨À¥g,?Œ#ڝ…"u?€ÕË/¨
?´Ý¯µÉ[î?˜NýšSM2?ê¾~?f-?­ÆÊî˜?™_¾r™ŒP?ŽMŽç¥¨Ñ?ĵ8¯5Å?«yÍòèÕ4FGL J0524.7-8304?ï3Ál÷À=~¢‹°£À:Mó™À0À<Tˆ'@>Ãز^7@ˆ$&Oö?ÍÛ·`Ô×?Óù|ƒ3Pº@ÿÞr¿?ü÷f³›x¿àHksì`ç?íÁú@£^>¿àJÞ˜–¿ë;›í0ðc¿ÚED"ٖ¿ï÷3rôcUNASNone?Ʇ‡uН?¸8@›fÖø?£ç՛E˜? ýg±4…^?À‹D{Wu¨?µ	ÚQúŽ×?ꪌI?»h}Ä°	?¨‡•é…?¬é'h'ä?¾h]²¿>?³	â÷?‹D?åd+·'e<?®m¨^'0²?º2q·"?žÜbq‹â"?ÍVCiÙÉ?§Ì÷Ô­]ô?çÇ õv~ä?¨îép?±G_´?¡WÀäg"n?È?ñ)v<"?¥~§GæP4FGL J0527.1+1152¿é¶s'i—À)[	¦qï1À9Ó@ŽeˆñÀ;¡¹ìxk@Ì´äxºý@‹®9cÎÜ?ÇV†
JÁ?ÈB¡û'Ýé@-©¼&Œ\@*ø==ù¿ÏZ¡¡¥×•¿ç¨^žEû¸¿çâJãS!¿ék8'ŽºC¿ì.4@ylÓ¿ïÿPþU0UNASNone?êeÏé+ýÅ?»8Ñ€ø?œ'¨Þçú?¡«•hœB1?ÂØkWt+ì?¹ýœÝ?ì¿íâ`?¶8ñúÃ,?"áP›â<ª? ‡ý}j?µôiö½Õ?³lSúˆw?å`1ç)Í?°Wh°y¯?°†±#³#ì?•›¢òãÿ:?ÑïèÁl?­Ç^91Õ?听ZôB?­º&bÙCÓ?¡`£O§+?"«Pß×ûb?Ò²'Ú-†ï?­'r?Âï4FGL J0527.4+6647?à
ý!ÜÒ1@1=¼#1]À:ÄÑ2À<¡S¢>"@›_-b
ç@ŸÅoá9?Ãaó$¥PÝ?¯fÿ0ø?ì(›?6 Î?ù÷Xÿ ‰£?ãÞDno¿à_0?ÿä	äO QD¿ßÆæ#5U¿ß¹"@"DÆ¿éÇaS/UNASNone3FGL J0527.3+6647?îM	w?Ûß?³{j2èr?sô蔜m9?{2ìn"?¨°Ëyn´g?³ýȆñU?í,ºÜ&J°?±²vFÁ/À?€…·uÓlj?"Æғ~É?´‰r0<ð?±•Ä·<?í¾>Œìâ?'ùˌ?€×¦f>º?p,Å¥ðÒ?¯æ5]¡ƒM?''6ÒúfD?냢›5¾?—Ì8æÜõ?¡@ ÝàòP?‡Qc'ùÜ?»BŸL5Øå?˜œ²ÁEë4FGL J0529.1-2449c¿Èøч
•À<b›Zcù¥À:µ¡qÕ/rÀ<>ç;
H@‡0Á¾Ñ·@2ÙÏÏ?ńΆý‹¿£<§%Hcò?ÜjyMÉ·@Tgm˜Š?Ù©,߇¨¿çÑxÞc"9¿çÎ0_C\v¿ë]H~u|¿à@".þñ¿ïöÅ>cUNASNone$?&¡ÑT?‰x'É/ZG?TbsŽFÃ?O¹¹–Êì?"ÊçåÇâ??ˆ­çú¤ºi?ïÀ\3þ?¡"dçE'ô?QÀÐ+š?dœdú5C?šëüWvΤ?¡½†"¸?í×g[Jl?—†';+C¿?z'
;¾Ò?køúˆoö^?¯7LÒÓ
?•övËÇõ²?ïM•«¸?y¼Sb£—?Sݎìñl?GF%‹È|§?•q«Ú0:?yœ'™(o4FGL J0529.9-0224¿ÌiºÊFÀ32 D®…ºÀ:}å‰\4´À;Än@O{h@öE)B@>ñ³/m@ӝ_÷·?êt™=SH@²ß­*p@ÕD¬à¿ÑGËÂᑿÆ|ÊÌ¿êw½ü¥X¿ïW}_§/"?Ñ|#ý`='¿ÆNxÉjl°UNASNone?è¾¢;d™p?Ç:èÞ¦3?¸‹àü»î?£vH÷n?À¿ï¡ï<K?¿]@ö¶Þ?ìm@çQ`?Ã?~ñv]¸?¦JøËÆ×?¹ÛéÑbû?±pƒ'âs?¶æ2çlÐ@?åî¥h{X?¯k²˜teT?¹X±à²?¡"ð®ûî?˙®N¹T?¨y'åËü?ìœ-÷s?Ã71~"lx?Lè?‰{=	?zŒJum"?ºäÇY4Uï?Ã"u§³.ñ4FGL J0530.0-6900e¿ï¶'ý6·À@:r2LƒfÀ7Öl9äþÀ;;¹ÿk@âQ—ø.Ð@ç±|å-í?¡š'_`D?•¦çÿ¶¸?öÛïqµ@±µ›ã÷?ìOu¹Nk¿Ô\Édb€(¿âµ†à‹P¿á×ÊÆbP¿á"€ãÀ.¿åpà<4dUNASNone3FGL J0524.5-6937LMC-30DorWest?â›Ò=AÈ?ÅmŒcÒş?Ž²í
•ªq?‡ #Ï-?ÙÒÄ'?ÅL¾ìl§:?èH\­NÁ?ÇÜÊëwòk?¶jyBÄ9`?¾ìŒTúÕë?éQè¨P?¿Šè)תt?×KWc¢þ+?³*H#Ý*?¬U‡";3?•Éj¯¾?â•E¶=7?³"Ù^Ř?Û*U¬d ü?¹*yò;ž?¼'ÓÃ$X?¥ÍÂòþíë?ݱ5bÒÞï?·94\ƒÛ4FGL J0531.5-7823?Õw¬5ÓwÀ>…'¢xæÀ:½ÚgüÀ<J=k›Y@ÿW±Më@QÁ"³¦‹?À1{¸ˆD¿°z_þ©z?ðÀÔÜeÇ@õpKAœØ¿Á© ã9öœ¿åø þ¿ê'%ëbd¿ã Å®¿åAÝ¥¸?ŠñTŸC
UNASNone?îûiÍÇd¬?žû
kÍò?gQœpR?^¿}°à×?°|…`1?ž§G+(?ï.~/b¥?œúöÆÏý?O;}è'äq?c¬PÒ''?™BÔJÏH?œ³yÀû.?î':–}?"Áğý¥?v°4•Rž?f–´¹]?ª¶PTƒË?'nl"új?ïQÕ7¶è?zÛ¦=—?X-žŠ–¿u?J§_Ký®Û?"B4·?yÇbH»Â4FGL J0531.7+1241c¿êè:Hr¬èÀ&Ž·ˆ—é–À9Æ2Ôh£À;iÏûUvT@Š¿šàª@·V¾È'?ÐxR!5î?Öܒ½‡_…@ìÝÿ$7î?óᣖr¬?ǯ.–ÁM¿èrd×-©¿å—˜Ø©yá¿ë{Â)°¨¿ïû¤üۈ?éÛG¹ÒõUNASNone ?Î7ÏT:?í?ÄÀäiI?"®
v\
?¤ÑWüÐ?çԛÂ-½%?Äæ<—Ø?à1Ýìå'æ?Ñt&dRãú?Äó줚Í?ǔæ>áÚ?Õ"MÓçu®?ÍYZ@þ?Ö£½´T®Ð?°Œ~}_?½³[k(HZ?›+B['(@?à÷µ¸pŸŒ?°*'*Na?ÃtYµf«?«!Ï^öR¦?¹%ϺšVâ?¥0,"œ}N?çþ/›HÛy?³"kŸ·F4FGL J0531.8-6639e?ï?Ìw1÷À@K´¢3œÀ8ƒE§©ý•À;ŽÊw‡öÚ@ÚùªPv?ÿɌ;E‰?¡þ¾›B!?"‹|ÂÀ¦Æ?äˆô'
´@‡ÒFß8?¾
è¿×È¥`LEÿ¿áG
À²ã¿à+7GMœ¿â†òÍèU¿¿×Ôþ_
UNASNone3FGL J0525.2-6614LMC-North?적Wnís?±¯æbI@,?l¾‹Pá?gÊOm¹&?ºÀ.þ?±mÍÊ®?íʨ‰å";?²¶©¸Ø¢<?ˆtÙírv?ž3PÊò0´?­8@æJÔ?¬~YI»?âÁµ'	°?µ
ˢr{?¢ô"™n¶Í?P«|™?ÙaøA°Å?´;Õ"!?éÄP‰«'Z?­3˜P)Û?ªaNz` ?˜G ÁXCã?ÂVj:¹ïñ?¦ÛwÉšä4FGL J0532.6+3358¿¹:;éyÒ?ÖâЯ°\TÀ9Õ¦k93þÀ;e·ÂyŒ´@Fj(ìç@'¼!ƒÞF?Îá\PãÈ?ÅФ®§?ö$SN[®?üÔ!s€¿à…°¾¤@¿æEMFÚ¯ä¿éùŒ|z¥¿ì}@"Ó¿ïÆa®pÁ3¿ïÿWƒuUNASNone?ç@9‡êÂú?ÃՆ5ԍ&?"ð㶊;?"ËåqD•?Ð@‹Áïh?Ãyq?7²,?ÜPøådã?мî+'†Ý?˜
	šæð?¦T=æX½¤?á3@vŽÇ?Ð͛¥ð1?ÜÛ]-Â?¯ý>'ÏÌ?µøëHÃÛA?š	2fÇó?ݦh¡ío?®–Dz;‡?ᗕ"á>?¶¥"¼>´?§É!óQÓ?'xe8Ό£?Ùװԟ¢?·O)í÷gÞ4FGL J0533.6+5945?¼! Oðr@,UîþOü˜À:‹øÇ&›À<Y>Y#@"yq…ÿ3@I©¿Š¯?ÁczcHyÁ?äF]²b¾@©†b…0V@ÐÎí
Š¿æSø`îW?ʊˆD1³+¿àKý"z¤¿ëÑ q$0¿ïÿ®2D¡?Ô¶0=µm5UNASNone3FGL J0533.2+5944?šµ(>Šô"?—(¿¦ú-?펓Ⴟ?°A¬£ÿ0?©¼-ȎŒÞ?©2''FÖ÷?¨´‰44P?µ'>m;®?ëü·!CV?Á&ëµóâ›?³À[É®¤?µèV\‰vh?³ÓœÉÏØ?œA¸HŸ?éÍUÂî?©Ø¾+dÜ?Á®üG;?¢Ïïõ6Í?¾ƒ/ü#!?¢ßÔç˓?ç%Ë1s?±#›d=Ä?Ä';ù(©?§"Ã¯?4FGL J0533.9+2838¿ïz)âҞÀ¤ì¦†çæÀ9@¹çíºƒÀ;!ÂÀ®@ƒvÐ@	ðÉS›‰?Æ*<Ó¿(ÆÚVM?Æè6 %#ü?ñ9"õjÑ¿á4PŸTÄ}¿åi¤ßGú¿ê#OÆðé¿ïúk _pÿ?í®/ªè¿ïÿ«±ÊUNASNone?î(¶ÃôÃ?²s×|ô2?y6.ñî­C?žãQ8Ljƒ?ªMÍñ²Þ6?¯Ýt¼¢×?ãJ9"¼Ts?Ñ$$óM@?~€Ôw"Â?žÂÅ°Wú8?Øñ‰¦exÈ?Ðã(š).Ì?ÚÎ×^±­?¯oŠœ?$¦?¼7ì†Ä*%?¤•È­c?Þ#-Ho?®Ómþg?ìLŒ aÂ-?¹ìûí°}?a¼«—Ç`+?nŸ øçF8?½
µ 3³œ?¹à^˜5ÍÀ4FGL J0534.0+3746c¿xq\·Ü"@4òd/UÀ9£¶"|#gÀ;c¬sßÌ@þ©éèß@ϒ¯šŒß?Í7ÿuÁx0?¿Þ-G#*?õ{¡çEô×@	©f®ƒa¿à˜›ò9¿çò³ç#¿çCKK¶¿çùš‹1!
¿ïûdŸç¼g¿î<Ö 
L	UNASNone(?îÅ°ŠÇq?¦:³Ú= ,?Qóäû7?WùÆõ[›3?£X=«¯-?¥¿ÕË#Z>?ë¤þœ8ݏ?Â`1ŸÝT?o(‰´"âÏ?‡ë€Á{Ï4?ÀïchJ:8?Áõú|8˜?éìVM'àÇ?©"TZž'?—#כTí?…8Œp£?ÅlâNÁG?§s‹îèü]?ìÃ3ÞMº?¡@A€b¡V?q"?¹Ô$Z?]QÎe2€?¸ÏšepOì?¡&Nú¬dd4FGL J0534.2+2751¿ëÐ/@ÆèÀyž×ÆûÒÀ:e:V=#wÀ;ÚØä2D @"&H?"?þ
Ÿu{­ ?Äã׫M D?ŽyÁô?ʧÓC3†j@0a"šK?Ö©Ù‰s²¿ì+º~¯•?Åû…‡hêz¿â©4wž¿è
ŋë›?Ö¸qËõ6xUNASNone?Ô9\­¿Eø?Á_œQ•'?p´ü´ÐE?eÙ{–úX?åÁ篶¼î?Ár~õ:&"?Ò©þIθ?Åf»lN©?o½KÔ¿(?')̈́ەE?æŒbCCå?ÅG0âëño?ä9朔+N?®ÑRÀ™\?)ëå²Â?ƒíŒþg"|?Õ¹"‰N7?¬½®îVB6?ÜÈC}`{‹?³—¹j+x?‰—¢¶'?¬ìҜ£¦?á5›âÇSb?³ë4¨¹Í­4FGL J0535.1-5422¿Í"ÿU$
•À@XÍJ¡À:V¶~¡ÇÀ<LtÎ6/@ÁV-ßi@qËa'Â?È;v8@Ž;?͈Šèü®<@]GóÐG?þvyÇQ¿åèÅP׉¿èaÊsc¿ãèS;wG¿ä«Àb±%¿ïÿŸóOîU¿ðUNASNone?íÜä]'fO?¦_y
@ß?Ä3¾/Óß?‹°ñýq?©Ï GÁ±-?¢Ä8øbô	?é¦.º×Lü?½ä6Þuã?©³Oû?©9{Éèe?Âú"À¾Ë?·ÿf~ìåV?éȲ²N&'?¨oÛ偣?®´šïÛw?—ã½Ë¦•?Á0zТ?¡("±'›?çLKqä…?ªÆj:QL?²ê\F'dï?›¢ª¸0òï?ÉY¤.‡r?¦zÝ+¾4FGL J0535.3+0934?ê3oәçëÀ(@ÛH'ŠÀ:ìÏ¡"cÀ;•HFÀ®±@ÜѪF@¼mFTx'?Óœ"$'?ÝÝÒä>š@ko\¯-€@
kSù&r?Ñ{,܁ö¿ê5†öÿ¦¿Þ¤Cy|n¿ë¯
Ÿ$óÕ¿ïùu!j2ú¿ïüZžÜúlUNASNone?îgm¥ÌfV?ªdùØü_ß?n›lö?sÿC[/Ù?§ŸnáZ9?¨õOA¯üÂ?香;Ë×?ÅU?Á¢²ó?™ÄPÁ?¢é'çÊٗ?ÆDÃ8ø­q?Ä>|L8F¦?ãôC/˜ ©?°÷…î±ù‡?´l퉳žÉ?™Þ¿»ã?Òü>>bÖü?®\#h°•?ä‰Inÿ[
?®Š»–Ò²?›eögË·F?†ÓvåÇ4	?Õ7
»"Žq?®mëuOÕ4FGL J0536.1-1205¿Öó;ÚTRpÀ6îיåÀ;\ÈWóÀ<†	g‡Î–@ K‹&5è?úV.u^Pî?֘"	\ ?å,Ýُ~@S1B˜+?üšÙ4ºð?ïÿë""i·?B;
ó?­x®ßÉK/¿Õ¬·¶Ì¿äTïE™¿ïþõU9UNASNone?ï­SVË?œ!õizÄc?w½«)Œœ?xIÞ¦Öϸ?™Ð‹1ÿ‡?™'_ÊrÖg?éµ:¿µ?Áoð^=Г?³¿›Û?¶óŽÈ û?¾ÖjûK7¥?µåð¤¡åD?ëÿ!B­r?¡ž…Ú=?œ(Ûuò°?Š¯îð?¸ü¿µèo?_¾¯{?á͊úç?³g¯ò¤Øy?À™È¶ÃÖÅ?®]æF¢ï?Ւæ	ˆÐ?´1[tbq4FGL J0537.5+0959?ë–^û|ÒRÀ&î™côÏÀ:#"D¾ÂÀ;œž%"ü@¥¾K°9@1·'¸¬"?ÊLå`íU®?Â*LDQ=µ?õ¸ÜÀ_×@"Äõ=l¿Ð]ó)®¿ÛëA,:¿î]©"â t¿Éíp†OåÆ¿åc¶ž78&¿ïÿöµšUNASNone3FGL J0537.0+0957?ï5€í}ó?£]Žœîgõ?PT	³ìµm?Q˜}ú@
ì?˜J¡Âñv_?£2'¼´Që?îÈÛ«Nz8?®Žžá7$?EÕâ•"ž?`ÌÎh5ýç?£íÀÄZ*?®I'¢]?ê`±Ç¶$Ù?©	}~y?ê~Vy÷?"¾•¡".Ã?Ä_écý^?§"µ0l4?îs~XPe?'`Ýí¡?g߄ÜAæ7?]œ:™?§P_̶ÛM?'¯3ãöÖ4FGL J0538.9+3549c¿ê7è ú@x7~òNgÀ9œ#…}ƒÀ;'<ðKW@\лnÖ@ ‰…O_º?Ê2(œ+o?ÕO´þÏÔ>@é>›A?ÿMðbF?北'·Ôî¿ä‡%"Ï8¿á&caNN˜¿ê^á6çÚ¿ëE¿&ñÜQ¿ïÿm²æUNASNone$?¬†Ùwh? ˜µ‡J?Ä°?+™í?À—¨\1Kà?éÓ{íH?ÁG×Ô«Ï?½J_ƒ}e?½
ÅL©›]?Æ8}'¤s?ÄPØ,u?æȔªç6—?ÆìÀù¶?Áû•'óöš? ÙDp?Æ9&('5?¥
a¥>?åüU¸Þ?«"²…—??¤[&h
^?…;#(³	N?ÄǪ/O×?£«H51	?é¸Û®óZ…?¤}³{V'4FGL J0539.2-6333¿íÊn= IŒÀ@	d¾ÆyÌÀ;$Æ>=RÀ<Æ<üàÏ@<YC=A@0:û~'?Ë-‰ûìÊï?¬a´Mzª?âùaíÍÎ@zê,>¿ïþøÞ΂?ïØ#½Ÿ]S¿ë=nöWá¿´M"O£¿ä5o¸õs¿ïå`³IUNASNone?ïÎ
èPåÄ?u'¢
8¯Á?3_K2ÉÐö?-‹cà¥öu?wė$`€ê?u;p·qã?ï"‰µ?'NÌ8@?4ÀÙú5Ö?JÊõž3WØ?ŠVñZëH?ºü
ÿ?î(«ð¨Bä?€«¾V`E?r+õé˜?_ª©°þ½?«/ÂR˜´?‡}êÙ?ïraßh‹P?x¨Ì4æO?c&q
³æZ?VޏŒ–šj?Žëã02Œ?v7¦¥3f4FGL J0540.0-7552¿Æ Æ4À>•#¯1±À:J ˆ5ÄÀ<Kìåq	@95:õIn@V—kÁïú?¿ƒ˜%{:?Ì#îX^¼@

òzœ@	N'î['οt—ˆŒî¿×9_\±Ü±¿ä/µš &¿çÂâh?"¿íÿ8$3»ï¿¨'õ:ªúUNASNone3FGL J0539.9-7553?ëŒ8likT?²d×O'Ÿ?¢kËh̗Ž?—×
×Uq'?ºhVèNY"?¯®ÔÐ?îD'ƒëi9?¨Ž]´	7?uC­³ºà?€ûv)'¸?©r2õ?¦m'¹¬"ß?ìï¨(ãý;?¡'¢=Ë?£×¡WŒ?•ÿ?R[2j?­-ܪ 6?"ò£ŸàÁ?n?Š' ©QC?ƒså訾÷?k¿Åóp†?ª
Žó÷Y?‡G+ÃÆ©4FGL J0540.2+0655¿ìÞÂÒŠÀ(Ü6q¬À:µ|8_ÂÞÀ<<3Ð$ë@!¼;ž½?ùcㄟ6'?׺àK}?ÍèþNe?úÔg–NÝ@[¹'ï?âˆö~vþd?ëȀB_¿âîà]Mc¿ÕmE	­¿ÈƒëÝ^?{¿äK™[†9UNASNone?íéG:á¿?¯ô»U(?wȓ"/Eõ?råoiž?¶T,Œõý¡?¯)VŸ.ªØ?îe¯ zn?º÷
bâ¯M?_Œô?yb7
Òà?®¡´ûñ‡?º¬œZ"HW?ëçvžÑôÕ?¤=ÃbôÿÓ?"w²Ö¦¾ ?x…ùÑU¯y?¾5T®›"?¢ëFXSì?êØ1dÔ«h?¤ÈÆ«Ü4¿?m&Wª[l ?hv7›w?Ä*¡äª?¤ä:FLê4FGL J0540.6+5540?裗y%RA@)ægrÕàrÀ;u"ÁËèÀ<VòQÁ"´@s"à?@¥vjNR?Î7'^"´'?½¦ù>ì?ðÿfèle"@@o7›LÍ?íc\%šÄ<¿ÕgnÙ÷¿çùƒCì¾Û¿ç¡Ó#þâÊ¿Ý5ý''¿ïÿÿ)@k*UNASNone?ï‡/"H1?…#ãïûO™?Víozl%?Pñî#¯0Æ?‹Vlþ¦%?"Z_}L±?íɵA´;e?µ¬t°¦>?p–$™rl?"V|¯£h?°±Œ°?´×Ë(aé:?í¸–¨H?–o‹ªm?O="X?t;ô£CJ?° ÍSå1?"b‰†ã?î§ÕúË(?†ý,‡ù®?jâhš³I
?\ìœE0N?£à\¨ï?†Dw¤Ñ/€4FGL J0540.7+3611c¿ìFz
»£b@}úâ~À:Ç=@Ó/À;dS‹'@'Œ`÷@‰3¿Â?Ðǎß×@™?àtüÌnØü@4zøÄ¢?ù¢îA'šÈ¿ï÷"}~[?ïÏü'$y¿á9NÖ&é¿ì3шô/è¿ïñò¡ų?îÞëuUNASNone0?ÆI¯‹–²?ºMOÔPh?¿<)‡'?¸</…¥úñ?æ†l:!?Â{"`ÇE·?ÀÌÃgø?ÁÁC'~´x?ÔîM@êBu?͟üýÔ]ò?áUØîÅÈ?ÎC"–·Òü?Ä¥ceX8¶?¢³VíŠ?ȅáðÍOZ?¦iM§Ç§"?äµ.ªvü?­kM)⬊?µ¾ßsh?™+ÌÖü;^?҅}nŸ«?µW{+ì?ä	lÁÆs?¶ß[ê¢I4FGL J0543.5-8741?ÙgT®—
À;ÈCރÀ:ÿƒ~`À<h30®ôu@M²³ñ߁?ÿžÔ¼…Vì?Úp™›&?ÁD°E­‰?üg+ˆD@×®7`iw¿ã}ú»×\¿ép|4.ö¿ß5ßJ}Ҕ¿Ø~ÿlÅ¿è9¿¾ëc¿ìA\[ðlUNASNone3FGL J0542.2-8737?î³*«'?–Ðo! þõ?sÆ[×Õé?p«6*¹(‡?¢m""RØ?•€)³ó?ï99ÐN?˜eÚå'Ò?[Ú=V-ÝË?iÛòÒr!?œ[4ðšXy?—‹G?O?íEÅŽÔ?™ë^ó2Ç«?‡yU!rD?}åá®ûQ?²äO/hQ?–O<«Œâ?îE¾Œ¬Ô?ŠŸÝ ZÎU?Gs™ÈK?kȽP«?§R:NÍÝu?‡ï±w.¹4FGL J0543.9-0418¿»ÆóL›íÀ0ú;%oüÀ:¬	æ~À;©Jß!c@¼Òo£üÊ@‰4\(?Ì
¾±:u?È·~Fï"@%cµ±þ@à™+µp?ï¿/À·ë"¿Ù­ÜÊ5ï¿éŒÏƒ³~¿ædËÇOh¿ïÿò"²¢?ïÿ9fS0UNASNone?íý8X­Å¨?¢ÈÌ,ºZ6?¨XÞK*¯?‡TZè!.Ö?¨Bd=Úã? Ëçùv?ìSÑôÆÑ\?¸ÑNa¨ÆŠ?¡êò8T?«¡`T&;?´k÷=Áëq?±Hh€7ö?äaLôäh?°gpïÐ ?²("ê#_T?–ø•®³{)?Ò³Ö+_Z?­ah^®?ã$bz."¨?±OyxFY?©h*Ù[8?'µuΩ=?֊5°wq¬?°'®ÿGÌ4FGL J0544.4+2238¿ïÇZÄ¿®À3F~i'À:YËUÔGëÀ;ˆöšüp)@ )¡n@Ø
±?ÄóÈd2Y™¿±{PƒP,?ê+Xx`å?þ(V˜½üz¿ëþ¢1ìÞÎ*L…¿âÐÞßôǾ¿äXxœÉÏ¿éÔç¸á]~¿Ð³HAbJùUNASNone3FGL J0544.7+2239?ÀH`¥þ?´óIèW?Š8Æ¤–?ˆ•ÝTi×]?ëƒrô	aJ?¶#9&`;?Ò…û"`?ÂÇbí{µ³?zB·hÍt'?‰Íï%ë?淓dØf?Ÿð
—N{?י1wNÑc?°[བ?ªÿ‹>2ó?*ͼ‹Öq?â'çK¤´?¯k†¿C¾?ÔtËʈ°?²Â¯1³–?Œt¨*áþ?ƒ.*¶Ù?åS"H ?²í¯"~.4FGL J0544.8+5209c¿í‹hG"d•@''éÌ·ÔÀ:´4osUbÀ< ÇË)_@<Ä~¾Ý@õŠžT~?Ȥ֎—ˆ?¡ä´Âa[\?Ò6§|0R-@9ÌÕh¿á_ç@ìYZ¿â«Ûmi¿æ/Pà˜0¹¿ëù=í¡Y¿ïiОh‹Z?íÚ¤ü¤*íUNASNone(?ê÷{ä®Ô?»*yã
zX?…$Ý#Œ€â?€	"ñß\?ÂÏ›çŽ?º†7ˆ^l?ìºî}Hß?½Ü–H¿#?†úa£æ"¼? 
þØ–—?·I?ßxèe?»`mžzȋ?ëgä¢(]î?¡|AÁÆÂ?šq=¬¸îN?ˆx–?¾$‹ƒŽÕ?ç´Ón?íf1sZ?œøÙ?xwÀ?wFÚ_։?i"2k5Á×?³Zù™‡Ã?›ó»ód.E4FGL J0545.7+6016¿Ç;ÝÜi¢Ü@/yb(D€À9Êãv\}¯À<P•V=ú7@Hñk<¹ð?ýHÅ¡_`¹?µ–…=5÷?ӋÄY`Äf@çíA·Zu@Ç=˜^?ïïÑ|^ö¿À4âµÂD3¿Èô±ë±¿à¡'A5ª\¿ç«
Û%U$¿ïúo!ËׯUNASNone3FGL J0545.6+6019?ƙÀ7£Kó?»=À.?é
Ë@þŒ?¿Õ[fˆn4?¤¼Mýbçq?£'Áž?°xPm7ó?°¡QêÒú?éÔ1:ÕÏ?Âßa™îb?ÀsË/^Ê?¾¡»}ݵ?Ð	›Ì#ȱ?°w¿yM8X?ã~mþaÐ?´<¨D
ÌG?Áôv¯¾ç`?¦‰Bà1W?Æë/?£üIšÃà«?âkš]Ë#?±LМPõ?Ð&Âvô$?¨›¢Ò4FGL J0545.8-0905?ïÃ4ô»À2­«ÀãŠ~À9Ó
ÙwÕúÀ;‰ùºk¡9@¥Þ^sS@Ð$ ?Àô+uúƒ?¡Ÿbûþ?ãÒácÝ @«ð¥oØ¿à~‹ì¿æõÊÝ^jo¿á>Nàð~¿äx6½¬Hs¿ã߃VR¿âñ+Pæ¢aUNASNone?íE{ïẎ?°4H¡p»Æ?o>X[=?išê8PÍ$?´Ûþ"vØç?¯ìt4R"X?ï3(E‡F¯?—*QËÚ?U]Óé:?euƒxšæJ?˜E'1å['?–ZìµÓ?ä¯DËØvi?´}6
XL<?Ç3®;|?†{¡K‡•£?ÔÅ7$/v?³&Øè\Ü?ènÄþ@Q?¦ÌşIO•?~tPÏ@Oœ?lo?÷‰?ÍQI€"¹"?¦¹È>"Œ}4FGL J0546.5-1100¿ÜÎÿ"À3U¢Æi}À:a՟Ú%{À;Þ|2€…Ì@'Áºõà@"ÕN´™?Ñh·#˜5–?âý ⣣´@|FØ+¥ ?øwÛ¿ÙþŽÑ¿{¿¸Ù"ì
"οêEœVã;¤¿ì­Z˜¿áðk¢æIv¿ïùOýnUHUNASNone?ÜeŠ;F¾³?ÆՃhs7Ø?³Âöáˆã'?°|#ʒD"?Þ©¸Wh?Ç*›.Av?ç&VNrá?Ç:¥'Ùý?Á	ŸbW_Œ?ÁjoE'?Â]hnÔì?º0Ur"د?âT4ÿžp?¯Ã8séx?ÁU¯~^Ö9?¢5xiœ?Ò¬¾A"'?¬s9ëŽL?ÖYÔ2³õá?²B©ûç²?ºâoÁR?¦±Þ]Ò p?ávÈ­Óe?µeÜÌZ¼4FGL J0548.6+1200?ï']ªô$À -i ­ŠÀ:3v†ojÀ;¿·lé7g@5XûC؝@³Ão1?ÏÚué‰?Ç6%ö4?ëÆxõµ#c@ú¨ïLÿb¿àóÛ>ªŠ®¿×ëD‡•¿êV¡'M¹¿éûibš)¿ï²Ô2ò›"?ÛǚþôgFUNASNone?çbdð¹êÙ?´יe—?‡(®if
?ƒpJ†T‹
?Ёð«@ùç?Â^ÞX‹ŸD?æWb¹Ãc"?ËbuŽC<ª?u®YȤI?ŠÀ×ÈÞf•?Òú%V§µ?ËÿN4½?â'Æ
-s?¯"ÏC?²Èn|´B?–AYFc4?Ö+ÂØFx?«Ë«c"³?íqs̞Œ\?œþ ªJÑî?wÙö_J˜ü?eðÕ&è??²öÂ5óŠ?œ.DÛ05h4FGL J0550.5-4356?áÏê>€KóÀ<ÿ‹&9O­À:¯ËlÂÀ<™TÑél@@ }7Š…Õm?øàYÜë(?ÓOÎ>¼Ô1?Ïsû$y&?õÀ›€úfc@}hLðô¿é«ç¿ç4=õ.¿æ=•W¹Ë¿Â…"¿µî¿â·{ây‡U¿äkg†ø­UNASNone1FGL J0550.8-4400?ï/ƒò¾?'¯ëßA—ã?ZqPŒÂÝ?Q'%ã@¡ì?˜h‹¬³|?' ÆÒM†Š?ï<ûw*!?—	Í Ì?V_8¢òöÓ?k3b<ä?›mëŒf?•¯¿ú‰?í{«Ù8+?—T¥ÎK?'‹*Qcs?u«ÈËOª?±Ñ;í©ÚÞ?" ž½æâ?íÞ3…CgÙ?'ïU;øõ?iò¤A²?c]Âá÷s?°>Ò೬?'rD_14FGL J0551.7+0446?é"e˜¾±À%î°t§qÉÀ9±*˜YþyÀ;…ùTTK@{"úX¡@4"Dž?ËO'ŠÝ>?á Þ'ö @w"}Š@£tvŸn›¿Á¯…,пÝ;%û'2¿ëC–ß~*¿êï/}œ
¿ð?ïÿÝe¡D‰UNASNone1FGL J0551.6+0449c?҈|áôg¡?•¨Àj)?È x~†^?À˜AtÜ	ì?à"£‰æ*™?Žƒ[lš?Ö'"¶ìÿN?Ì»©­ç z?Ö·šF?³?Í¢SºLö?Ó Ñ5ÌÀÿ?Ɂó`˜n?יTÚù²?°['³
˜:?ÇJ–?§ªÒ³Ã	¾?ÜØÚ×??¯*'
«ã?Ӗî6˜?²üWWú2?Ñ»³A9?´3­Ïy?ÛKVêIˆ/?µo8Pˆ4FGL J0551.8-2130?îUþ
ÇÀ6Yl6KìÀ;jlËÛ5EÀ<°IpŒZ@%8ZåS×@1¡šïÛ?Ñÿƒ
6?Ëàs±B?ö"ÐÜüÆ@â×P3t?î3Îc¥ÁÆ?îšcX"쌿àMªx.—¿êå"Ï7á¿È/ïÜÇ@Ç¿ïÿ~À¥L*UNASNone?ïžíæŽ5´?'ÎyÆ!ž?sÁÓ:t–?vw=çhüÊ?|Ç9~q	{?xõ>ðã/Ã?ïñˆ®÷¨?0ŸÇ¿?eÜs!2í?}q–Îu"¢?›FN[¼ä£?™~ ¬
É?ì÷ln'¿?™\üÃL?•?2Éj¼?‰dÖ|LhQ?²ôقgP?"‰`¾h'?îºvq_²Ç?Ž`\?JdÄ?v©z¢Ÿ?q¾?$1C<?¡–cº¬O?ŒÙ£Áy4FGL J0552.0+2656c?ï––/ô?Çh'œ&;ÔÀ9—ž™ À;8ûefŒ&@›Ñ,Wø@[œ›¬™Q?Îb~ºÆ?Ú	{>d¿?ø¬Gõb?ò?߉=¿ØAN^²½Ø¿ß1BªŸ{¿çeQÉ oâ¿èÊ/cšÚ¿ï.mÚÚ¿ï;^g"dUNASNone(?±µÜ¨uÈ¢?®qҀFÿ?~"!Ðò¥#?¢"…yàzÈ?íŒ<'Oa¡?±ÄiÆè?Ðj3b)½?ËçЖÑì
?¤ööÕ	‰?²{‹CfÑ!?æ{væÍÐÝ?̔"ë½Îû?Ñu'rhÃ?«vu?Ë?À77á=µ?œËÚQ	hÜ?ãD°øÓ¦²?¬¬"Ž,_R?Ñ÷"¢@?¾ÆÕ¯ôì#?®†p4"?¤
q¢®v?å2í®H?šú]æ¾|4FGL J0553.5+4810?è8ðòúf—@&HƒýP"À:—Ò+ìîÀ<¾mŽxÔ@Ö!·4à@O–áXu?ǁð/¨d?FÚ
Û¢¾á?ÿ	"=—¿å Ã6iI¿æ@š>Û"¿ì¿†]|²Ù¿Î£¼ÞLù¿ïÿýF\I?ïÿÃÏÎ	
UNASNone?ïÆ«¨ƒ°(?€®Ff'¦?nW–lZ?sÒý[€?jýSg¹k³?s¸QÊ|¡ð?îI?·<§€0?nÀýnÒ:?"§1µ¼j?©ƒ¶Wñˈ?¶l_³•Š?ê·-³Šßš?¥oyÄØ?ËVïa?Ž­RªÁ?ÁiÙí?¢ŒÑ¼+o\?ïLÛ¼¯»?ˆ¥ªøøû?gÒB‡È?bQŸŠ˜
?"j@'PNg?‡cžn¨)4FGL J0553.6+0100¿Ü ìr?‡À(¸mµ@æÀ:jíLŸÀ;¶3PdŒ@'Ù®¸»@ß	zÓõ?Ø^K¥Dóz?êCXz™@H¼¾aÏÿ?ý‡¼!ƒÞ¿Ð¯9¾èˆ•¿Ú"ã"Ê*¿è0‡‡H^>¿ï¼sÿP³?äJ
M{¿ïöÿ<
ÈUNASNone?â|T†,=?Çìû°ëOÍ?ˆÁ\$ 1?¼¾4v?Òº¦¨á—l?Åüöðüæó?ç<>9üR?ÍS­0Êr˜?»šU
ޘã?ÃjûµgÅ`?ÅAܒž>H?ÅÊøÚ3q&?Ü4ôÏ×dX?°aè)Ö?Ë£5ra´?­W½SÕ­Œ?ÕùpvèêÍ?¬ÓìøQˆÍ?ÖÔ.sg7?ÀÛïÛèÚ?¦V˜t\;?©›Æß5&Ò?ã0r€Œ1?ÁQn¨Fwû4FGL J0553.9-5048?ê-ý¾©•ÝÀ=ˆ2¹¯æÀ:æ9ïôÀ<³ªÉlÆ@s*ÈU™º@«`¼z.?Ë{O+·=ï?¹o0'ˆ?í
Ž>F·Ÿ@S—ÖJúпä¼ò.†%I¿ã—¢^S*¿æ»ÀÖ…&¿Âf%cf×¥¿î
?¿2°V¿ï' 
UNASNone?ï9		I÷¤?î*Oäáë?[¿M8è‡F?SsýG±Õo?—"ê2ƒ?SO·¢Š?ï|¯7$\O?Žšã?B®3Šhƒi?XÛêÿÊõ?©NþBd?F3cm%(?î>"5c•ä?ŒõˆÀ¥<?}6	É¢g?s^~Dsg?¨pûp¦-j?‰†¨dG;û?ïF*yÌuP?~	±
Z{?nScÜøîé?añý(8¤p?"pDJÒ84?{Ó2n>
4FGL J0554.0-0839?éÁ¦y¦àÀ0§õƒ¥À:yB¾ÁqOÀ;ú¬ûv-"@€ÝŒb¤e@ÿñQçSa?ÊÒ¥û|¹?À–Dû\­*?ôGòø°€f?ø>3i¹×þ?ïÿ*bT3¿ÝhLðô¿ãÊGÅwÄ¿âÅaôfſ揉	ÿ]C¿ïòd6
~UNASNone?쩾ЙKZ?®
-˃?vÖ½}ë{?r7["ӌh?¹PL]Æv?­XKeDŽ®?í¢eÒ?´(ä‡&Sd?'à>—T"?˜{Öqè?²ÊÝ1¾ÜL?±-Ï0Ÿë?éøuL—ö¶?©(äã÷¯?–µº!T?¹8ÇΝ²?ÅGˆªˆàÿ?§&žzÃæ?á=oÀš?§ËT2¢k¢?°9.âj	]?"˜©š=<Ý?ÙÕ: …üu?¨:¨Íù¾Ò4FGL J0554.2-0259¿¼BñŸÈÀ,'gn¤"ŠÀ:>zt:d€À;¾G^cb¦@%ï6¯©@ys{øžã?Ám6åtÆ¿ŒÃëk0™?ÌGԪ矷?þN9Vé?É@ˆÆ¸‹¢¿àqöó4¿í¦ÉB~ª«¿âê®ñ𿑶N[,Ìg¿ãêJŒL˜UNASNone?è|Wk0D?ÂsÆ  bß?'@eàў?g>o°Â?ËíºFƒÔÂ?Â>ƒ£HŒ?îÞêÌe´?¥PØÎH£Û?`NàöˆŒ?rçï«´?¡e*<5ü?¤ŽÊ2?æ¡íÞb?±kxúI_?œQëÓõ?‡GlÙ#?Ð÷…ü ×?°&~³¿ÞÕ?ë8êí?¨BL¢ÖÔ?kªÈv,?cfÍ‰-–?³–QÞu?¨š':4FGL J0555.1+0150c¿ë…h´
RÀ'GLnm›åÀ:F¹"À;£)¼'ì&@úîãøãV@ŒT6¸ú?ÎÕ1J?á@B,Ja@Çþ0òç?øÇøâªY°¿ëL§ãß8	?ï·C[Ÿc¿à;Vƒš¿ê=sº¿ïÿýç!é¿ê]"°§UNASNone ?Å`0Áv"å?¼®Ñ`Åv?Ϧ¶<(/?Ä©4ܤü?â¾FI"Tº?ÉÀ6e/?їÎÒµa?ÍÞ냣š?áu‹8ªà??ÑD_TЃ?Æú5wé¼î?Âwhx?Å|JÓ{6º?¥ÁéO-?Ú"®œõú?³¨\ÕrH¡?Û,•¥n©?±âŒt•œ?®¾•Ø¹l?£ZÛýî?Ý#uƒ´ü?³íÇDVÞ1?߸‰á×?³°ì¾o–¥4FGL J0557.5-4452?îS¼k3]XÀ;óìþ›{òÀ:g%¹Íì‡À<NØúØ@êç§Ä¡@t¹­6?ÂSÕÀ{ο Ş°.Ü?׍ÀÿA@špkø̅¿×@>^Šyì¿é2"²¡¨¿êÈx	&o¿â¾N"ÈQ¿ïþ
·x§²¿¶²$ÀS UNASNone?ïóŠ'"?X™`^?FBbëÉ]P?Gþ¶ÃY.¤?K""óÀUÛ?PÒØÂ`?ï‰çH`Hb?'/þUÑd?E'©W¬ëµ?\1u"V?Œ.RsÛ?BÀû¤éo?î‰,iìð?ù߶¢r??w"âٚĠ?m"¸åÎ?¤ˆÝÝØ\?-v7?ïÍ5XìâÅ?f`¤–ñ?\"'Êgw?Sxˬ>E?r\¯ô×o?a§ÁКb=4FGL J0558.1-2113?éþ"_4À4à¤ãy·|À:USʂo±À<jT¨ÎÀÃ@¿(Y@ˆœ|&Â?Ǩˆòß[?Ѓ­Ÿ
ã@÷9zu$?ýs$ºÊl?ìO"¢—D*¿ÆjOv`¿å—ö+jçտݗ|ÞÍÖ7¿ífNžHªê¿ïÿߞ¶ŽóUNASNone?é†@ïtên?¸Š‹Qj?¬¨žë磋?£§x'­Ùû?¼ԇ2md?´V˜Rܕ?éïÆy™-?¿-n¥Vp?´Z^'áHX?·èHeŸÈ?¼'m°±î=?±jš[7Rï?èu1dŸÔ?¬Õ‰f'Š´?µˆlï&GY?Ÿ;#†zV?ÃgZÚ]?£U':zÇ?çšÇøuµI?¥'"…ô^=?À3ŠôCÀ!?¢ø
Ô®X?ÁaU)åj½?˜~¬Å;B4FGL J0558.2+0132c¿Ø%­ÚÕ_TÀ&/¢ß"xîÀ:?ûUvTÀ;¨
^u×@žÒmö} @ÉzUý?Ôæ‰ah$×?ڄKßQ‰µ@
;3Úøßz?ÿ†xÕ~Í?íµ"Ód—¿ßƒf|`΢¿ç•jËOõ¿éŽ•¹:I¿ïÿÿ>¹ú?ïc!u´UNASNone1?Ýu˜T»?Dz,%t?©þ2µS?¦¹½ÇYj–?ßJ¡iAÍ?ǧÄa(e½?ޏ}³É?ÏÈ*šG=N?ÂÄöîşþ?Å
§rÉZ#?Øn™|8?Ì\c!,À?ØFF|V?°û{oÊ?ÃË_fv"F?¡½äÀéœ?Þ
H±‡?¯¨GI^×L?ώ ?¬$3Ç×Ü?¿wâÙ(I.?©Ö>Ãp?ä-[žqT?±*4Ëv4FGL J0559.3+0352¿æùõ±˜À#"Š½]ÄÀ:	-ãÀ;±6½+o@µðöøš[@-¾Ý '?ÕE~ð ç?ïÿ› 'V‡@è+}\L1@¸PW†N¹?ï[Û]‰H¿¹C`Á¥–¿îFÄ	¯¬+¿ìÇæîð
¿ïٓLØ ¿èñ$?¥\pUNASNone?ÖðìWíe?ÉG#Ôé?Än
n¦–?Àt<™Îø?ß\÷ð¿P?Ìí틪3?·b£e‹?ÅÔ]«ð>?ÛþòTªãî?Ñ?‡ÝD÷b?ڟ±úiM?Ï­­?ÚÄm‹L?±År'?Êï1w´µ(?­Ú%Æ)?×Ãú1!?®-×iæº?µãs[+?¢¸>ô`A1?å"V´ÖzB?½p87׎Ù?Ðs™¹|@¸?·ºEÃz:|4FGL J0600.4+4949?ïÃؐ@)ž™Ç¼Â"À:í¶ÓfDÀ<Jž6·L@ _Ž…ê:@´Å¤º_?È{T44ºó?¥S°ß¹ìÿ?Þ–¼f@Lyð'οë(øçÝÊK?ì*³Éƈ¿î\.Õ?ÆÐ{k0P¿é"3É[(E¿Þ¦ž9çWUNASNone?ítn¯WA?¯ß5L®ð?'J"Ù•"°?ˆŸ$ˆ¸3?²<ÇR¡§?®fÄð=î?ïy{˜ø–]?š¿øÅy?Q®t$XQ¤?j‰[‡ð»ª?kK=O^}?™@çÑeáÒ?ëÕn¾<í`?¢‹2ði£A?'üxZJÃ?¦jõäƙ?¼ÐJðK?¡Ó7?ï#ü÷¶Bu?ˆ¨ÚŒ$´±?{ÜGºAq?wO*jZß]?"‰O¶ þ?"4^rì¾\4FGL J0601.0-1016c¿ïN<»"ŽÀ/žj±NÂÀ:XÌ'©»À;žøÐ`Ö@¡di6$@
X³ö<2?ÏÇó^±ç?Ü®W+`@ü¼Ï(ǟ@Ñõ!T¹k¿Æ°(|Jÿ-¿ØiP{˜|¹¿æ£mùÞý¿ëá¬Bh°C¿ï÷íA·Zu¿éˆ²r®sUNASNone!?ãÚpš_?Çš~Í®Û?™u*,¯ï6?"33#Ê?Ö´œ|ÆN?Æü‰$Ød?ë،æ»Ó?¼kZCz?£©c®o˜?­
V¢Úa'?·fçCré¦?µâãÒY(?àâž	³?±*v›¦¯™?¼`©m¨‡?œ²†ÞÒÀ?×"™Œƒê7?¯Hµmߗ?Ûxli¿®?¸ÿÌ&y6?Ÿdê²ñ?ˆöÁCðO£?áH¢§]?º)±f$`4FGL J0601.4-6057?ï1GhIj'À=|MüãÀ:ò{+‰>À<'é]ýY@¼úh;~@VÁBU&?ÓBýwºw?ÒK!{û£û?þZ%zãËí@¥Šeôül?ﱚa•œ4¿èHâA©¼¿ãtŸM ¿áà1~'ML¿ïÒŠÝ>4?êpYddIUNASNone?ï9±!6b?"Ÿ5Þ¨Œ?p¨££g2?r׏'Ë×}?"Ÿ²ó?SW?'–íÆÕýí?íܺ
s8®?¨k€¨Ou?€T¤XyÛ?ŠE´¢p{?®6BŪ?¥l‹	›Ž'?ë"ÈV§?¡‡:y—?¥ô8ïÓh?'XQ$Ù?¸mÉӖº?™ä<³rm?íuë@GQ±?•ù<nGÔ+?‰*‡ "ÜJ?{P˜y¹¥\?±+U	Áî?"´ò—Ó:4FGL J0607.9-1904?ëK èá^À1쇇H^>À;-ÕctCŸÀ<Û®ïl@ b¸¬.q­?ÿ{ ÒÞ^Æ?Òâðe-VO?¾æÒ1›Ä?êÔë´ï`v@l´S"6†?ç¤ÂAÉy¿ídƒ¢·O¿â8j_oQG¿×Õ'¤´ªÂ¿ÝpĎ9ê¿ïÿ'þKÊÚUNASNone?ïqÊXß?'Œv(!Ô?Q!yŸÜ\=?Z Ü'åð?Ê&ì·q?'›"öPê7?ï	|£hb?DžL"?Z¤¼_Íæ?nŒ©ÿ¡?œô"¥šÖ×?œ3r¼ñã2?î¥^ÌÔo?O€_FÔ?pl˜¡iÑ?\¨yµ:Ýì?­(ÿ~ú?ˆ,‡º£Ö?ìpU¶`°?›øÇh?ndÉês?aí…Éܹp?»&¯ºO?œi¬ÏZ4FGL J0608.6-2305¿î£÷ŸšuÉÀ3SÐÚèÀ;LÂPrÀ<ˆœC˜E@ápÌÚ@‰ë têŽ?ыÝÄ@â?ÕHK=–
ž@¦±\.?ôV¥‹•Iÿ¿è8Eáá†î?ÌùÁâãåm¿ç=|'‡"C¿ÞùŞ…;¿¿ïÿÌ3IÙh?ïü,d1UNASNone3FGL J0608.2-2306?ï/"Á²o?"JëBï—?v"'‰È3?}ÛoPÑ&?"h^ªÊ?'¨›A²|?êÁf† ÷Ç?Àcä‰ZyW?«&¨nQ	?± ª!¯¼?¼aÊvÁI?¸?™/¯Ž?êLì0é?¦>ÌoQû…?¯zU´Æ­¬?––vœ¿M?À:#ï?¡S¯[: ?æ€w×rv?±5bPW(?³¸‡ƒìã?¡5¥ÒOþç?Ì!Üà­±6?®íÖ4FGL J0609.0+2136c?ì6d}ØóÍ?ì'ÔžReþÀ9·¡I'CŠÀ;F"ôï*Æ@itû)¬w@
€™îS/?ȑ)]œhV?ØLv›gÏó@ê^ã»&?ëKÿ‡V˜¿ÓmˆÄŠ3¿â²âÀÔñß¿àJþ¥·à¿èÙÇÚñS¿ïþAÿ©ÃÞ¿ïó÷H¡YUNASNone3FGL J0609.3+2131$?ÈÀ.k,j¨?ÑnX\u?¬Ú~ño\é?­‰øÜe=­?èLvïˆ?Ðý"ñtj?¤ëU¿µÁ?¯?˜ä?č`:&€î?ÄGîïôµr?éò•…Ôh?Ävs|;=ó?Á9oUïÄÅ?Ÿ™	köõ?Æ*Èþš?¢ô76°ìÀ?æ'8d)?¨«è°?œ¨Ý"Rz~?'ÂOxÎÝ?Òí£7î?µL®"SLM?å£ùAœÐ5?µ×[…‡S$4FGL J0609.0+2006¿ÎoºS‰¦?Åd†gbºµÀ9i'¹'m-À:õè½ÄM@¯r2!I@z¼i¨:?Ô;âjØ?ã]0'oí@³?…Q
9@¯upðX¿Õ1Ä{¼¿Úâ;Þ}y¿éC¿rq6¤¿ë*†ñ÷(Á¿ïÿåþÌú¿ïŒbUNASNone?Ó'¨éåñ.?ÁŸ7»æԈ?Ò=CÁ8{?Äk÷ñÃb?ڛTᓸ?Å«îY&x?¢ºàíæƒd?¢•äýuŸ{?Æ=žvp³œ?Áƒ1:¨ZR?éDêS…jã?ÁÑ_m·'?ÈdÔ»Ìgâ?¨µÉŽ?Î-
9.C«?«BcqR*?â[‡'ÁU?°¼´¸'q?"™ ûb_s?zTÐka¶d?Ø_4ä5?¹‹U57£î?ã3˜†
d{?¹fYÔ®}L4FGL J0610.8-4911?è£ÓÍO²#À:–YòºÀ;˜=Çá¬À<Ñqk}&œ@!A'±tט?þÐæòèÀH?ÌåÚ9òÀ?q£x}…µä?«ÊD /9B@=^Wú?ï饠ÿˆ¿êŽß+t"¿äHZ!^Ÿs¿Ì‡ì]‹ÌQ¿êk[˜­
¿»€@­S8UNASNone?ï·¥ŸÁÎV?~ÙÁñš‡?<
7Åò?5Ûz'JêW?6.QdRï?}q±g–>™?ïlÃÊ|…?ŸÝú¡"t?Cã»3J?U~M#€m?'Èhå–â?Ž—RÞZ—?íèA%å4—?"håYÇ p?o^¬UØv?iT
"À}?¯†à‡Y?' A¹n_­?î¹ía"/œ?œù'3?_UŒ›õ¯º?VWë–m±:?£f}ÝXÎ?À£@u»4FGL J0611.4-4722¿ëþÔü¤´À:ÇÚÄçÀ;‹ûZu—À<¿a¥6†@ý?Ãdn?@$	å\Ë?Ó«ãH9Tµ?Äï"77y¿?îü®a|ǧ@'Góߋ@?îâ<À县ãØöT…"¿Üß|Ò¹uØ¿èDÔ «±Ÿ¿Ð6ɀ<%u¿ïÿHµ{wpUNASNone?ïOs üÿÚ?Ÿ19(
?ZŸoÏ.‰?U["D^åH?"g¤ãn¡ß?Ž'8,5?ð?£s$Yd¨Ô?ké'ð]ì?ƒA"á~¬?¢¦˜ï/?¡Kìc¸hý?í ¥7ÕþH?"'ÇFê	?~@î×dž7?rª&ÆÎ?±ÇSÙÃà?'<j€—?î#º›.yf?'ýx­Ðà"?U÷Ib¶'?Q!!ÄIÀ?­œ½Sã?"ÆÍÉ4FGL J0611.5-2918¿ìé¤lízSÀ4ñŸŒ¨À;:Z—%KÀ<¸'MKã-@O'M ð@¼ù jn3?Æ
)#ºÅ8¿"zÞåËmÉ?ÐQJ8ˆ@!SYÄAŽ¿ïÿ_Dä?ïò$	ʄ¿èL?^9Ç!¿áŸ©³`ë¿âø›AåR«¿××Àâ¯bUNASNone?ïã9¢"Eé?e¢%Õm-[?9nÿ›\îû?5¦ì=&¿t?i˜}ˆNwï?dq#ŸzI?ï¿Þ3Zξ?mỆŽU?(ªØ0¸?B!;v¾5?KŽ?€ìêlŠ ?^é½Ø?‰×Íma?nuN!őL?bg¤\ÁÙ?£Žå/GÉg?ˆ._;a8¸?ï¬A–	R?iÙè#Mv)?J»v;3ân?=ym!q~¸?ƒLø6ÊmA?iA;_ÆA¢4FGL J0612.6+1520c?ïÊX5ÌÁ¿õûš—À9Òc+Hƒ'À;$ý
':@jüz9'@'BÛFã?Úð¬¥åØ7?݈Vü1Q@ˆ.›
³@ŠJÇ#–?ïiGâlÇ)?Ô¿tŠ˜¿êrÇ2Y ¿í¦grÕàr¿ïüsž]M¹¿Fz•ÈSÁHUNASNone ?ä¤k:A¬\?Ǔ=6É/?°FÏ3M§É?°ÃÜîÝ=?Ò¥u¾©=V?ÆÙ#U'W?¹ú»¸çÊ?¶¥ S׺?¸»B I¡ê?·¹ÎFÑ?é©V´®É?½Óósh—?ÊÅÔ«&Ìú?§8ÀBa-ä?Åxº†ö!P?¥Õ Ä5?ãð\3xÄn?®ASuöG§?´Þˆ»J÷/?™EížIª?Óy2ҀÚ?ÂIÀ¡N?㧕æ­`­?Á ¤'Ä4FGL J0613.1+1749c¿ÚûU,=†Ú¿µ¿¿¯>-À9T*:†åÀ;dØǬÒ@ˆuÒ4j@
0'|G?Ã1U¡Îò?´Fˆ"ùª?ñÓÿü¥­@˜,J¶²"?îޏ¢ŸÒ™¿äKb¿gßb¿é¶nfÔ¿éÔ¨c`øh¿ÛÅÓ~—µ"¿è{éOºRwUNASNone$?dz*GA÷°?·˜µ¼~½Ä?€n0$ãóL?xŒþ/Æ®T?éÑ|­›òH?¸tlIíµ?Ñ/Å=)®=?ƳU"YÍË?'éìTj&?"$è—­Œ?çu°~m?ÆǏq>}?ÒÊ»KO?­ËÜ¡Úç–?±Lð½Yª?'ô°U¨û‡?äqpÄB­D?®7µt¬?ڌë˜^F?µ˜~fš?–ŸÊdC?'Þ-ÊÔÊ?â']}ќ?¶€˜ÈQÅ4FGL J0615.9+1416?Â^4Ûпòê1ç٘À:!<ªÀ;€Uu}ZŸ@©®Œð¾Ä@sÆßî?ÒMyšöë?à/‹^¿@
9™Üµx@`¶™Y­Æ¿áOuž'§¸¿ã5­–¦ ¿âöT…"RX¿íχ\€3—¿ïþÚH¶R?ïùv
£V²UNASNone?¹óó‡½?²Úí|µr?ªRÞÙ?§«Yˆ‹$W?ëÜe>ZÎ?¸á°eâšú?Å·0¬ÈS/?à0n•Ÿ?¦Íü0'ʺ?¬R%«µ?é%TËn‰?ÄÚmv?Êÿý'éÉ?§g£š?ÄE̛¥à§?¡®œFÐ|?ä.t\C¤?¬{¢Ãlï?ʉ…¹É—?­£HË6Æ?¼" =?¥{C';
ï?åÚ®9˜V?±µ#,Pù74FGL J0616.5+2235?ì"JJZ@=õ~œ¾À7ÈE`\a*À9ÞÅFƍî@"ϝ"úh@R¢™ó[­?¸–¾»<,?¬ø@¡Žc8@ÂJ»5'@V¸­¿ïâ'x?܃ÒÝÝì/?ï^ˆ¶óF´¿Ú%р´¿â#πÜ3¿â"@^"àÍUNASNone?ºHã)DÎ'?íTú—Ä?o'iP'¥?y'qnëÑ?ì—R1Öª?ÃÁ•q\s?×AF—}?ÐåÄ\g:?±öi#úÀõ?Á©ŒÂ»P?â dL]\#?Ð}CۚE-?ÊËB©?°Á˜š›vh?©àM
*ȉ?–¿ÂGL*?ç¯5^¬Ò?±«á}ïÀL?¯c&ì5H?¡JãG ?›p@-û?˜ðÿÆeŠ?í1JÉ;;?§rÏú!h[4FGL J0617.6-4028¿îø`ÌQÀ7Kğס<À:Y:Ütà}À<Aß®Pá@"ÁlFz8@²c/
°?Àâ2d¬'¿~9¡æܐ?´Œ•z%5@¿ê»Ë?èQ­DqI¿ã–ñH­¿éŸK¿ñò÷¿í-­LÔÄé¿ášß÷-É¿ïýVlô!UNASNone?ïú‹XÝ?vR7X?2ê&'?mg9é–?9'#"jð?eûLao‡?ïËþØ­ƒ?ÄŽ=g};?,Ô
ï&Áã?M½VàùÓ$?yŠà<0Œ?€¿¯ ?îØú¸bf?‹+£Yî'ó?mGDșTä?eG,БpÃ? ›à*pDJ?ŠU«"b?ï釷Ç*?QÇÇ2_¤?%"œ¥Ç?±dóȾ?e&&ÿ!?QB·âu4FGL J0618.7+1211¿ì¤‹t¬"¿ùvœ>ˆÀ9Žé#D¨¦À;G5>¦-ý@ʈzdØ@5½ÿªo«?ο<"÷?Øwîý`h@ëð«Ï?ýÏôÄã¿ÒÁÞݢĿâT‡@сg¿ê±  œX¿ïþ†¸ìE8¿î{qZ¶.ü?Þ>;Ú¡¡¦UNASNone?ÑJFm²UÇ?ÅäyŸOæ'?Œê€ÉÈ]? nŠ~"Ê
?æç2Åÿ³¨?Æ9£©úD?Ìê"Á"oŽ?Èj·oÿÜ?©\'Ÿå2Ã?°.©¥É—m?ç/'µœð?É~¶…P3Ó?Ó©‡òº?°iwæsq(?¿Kõƒ^ª
?œÐÈÌ®¦¸?âA½ÂŽ1a?°­A{m¡?б
àFí?³ÔŽ*²|?·ñi–Oš?¢-+Hr?ä©Kì)¿†?·«Â§rx4FGL J0618.9+2240c?ég"*GYä@díoڃoÀ8£$G%ŽÀ:V>hñ["@ä-;¢m@0;>šo'?υŠX‰?×E$>MÄ@h›€úfc@ØçÓ
ƒ¡¿ìŠÝ"3¿Ù_`"T"«¿Ò'¾+I¿æO_žÌ'¿ëá'fw-^¿êœöElUNASNone4?‹—ÜÄ´€4?'ÓûÕõùr?ÜÆ÷èBŒo?Í·y°="¯?á.$˜ËçÉ?Íæ$`X ?¢[¿X'Á?©F{usÌ?à~ˆjl?Ð÷à‰Y/?ݏ‹*´Ê?ж´ö?¯Oopý¬?˜±ìd'÷?Ó!ˆDïB?²<:2í,F?äzDûM·T?²S€Õ'é{?…´í×F}ƒ?p%ý¡@¹o?Æ4KY&‡"?±'üÅÂæ?êrYD%?±"7|vÝ4FGL J0620.1+2246?èÁ÷îRrW@
º"¹À9W|i+À:ðÁëÈ:—@!`>Æ4W@F$<jÿ?ÄK©â,£?°Ø*ùÓÁ?óR¥ôñ¯?öí՚¦µ¿ïðÏ«¤^?ïÿ}ÄPýI¿è¦,Od¿àcuÏ¿ì×LbY;†¿±²à<–3^UNASNone?ÀD¨Î«ê?¶0
­ÃÝ?-ÄðÌK?–tý/a?ëmg¤Î¤?¸&»¶*?¿ã^[­®P?¾¯ƒ?Æ¢`ÄA9?Ȝ‰U'#¥?æ[œY9ç?ÉaÂÑõ?ˌ7'Òcm?¨"™žÀÑ4?ºY‰¤ØAø?ž"Z_B?åÑÀê°^å?«@¹—7{M?µ(úâÇð?˜ê"H8Š?¿¿´²æ©?°¨JQ3 ?ébê
c¢-?±sÐà04FGL J0620.4+1445?¦ðÊ¥L¢'?l`ÃËW"À9ªu߀-¸À;LM++ýµ@¸¹Å^@F&}BJþ?Åʤ¾æ°#?¼X̔m¶?÷pd·9½'@´Áº ,?ïÌÝÉtR¸¿ã¡fµN+¿è=Ëݹ"¿ç_™Ã‹«¿ãË£l2›¿ïÿ!}ÿ	`UNASNone?á[0¾¥ú?žˆ:Á*ê?uJ¥Â=«Ã?n.HyÕ?Üôsë¬Û\?•³â)?Ö
Áé^¶^?Èд)`›?zÒ¦Š×.µ?ˆ×–8?äÃy¾:ös?ȾdÍåÒ?ỐÜF@©?´Ïù«P?¦=vúÔ¡¢?Œ€Wpò?ÙÁ/hêy?³"êàâñ?ãŽê‹n…4?¬¢àº¯ÆQ?"²"ÂL/?yF®zÊQ"?חœþ3Ô?¬qº|rBª4FGL J0620.7-5034?×®NŠ°%UÀ9Q—ÃքÀ;•æR¯Ð=À<ä1Uãad@!s?Lœì?³IWaæ¤å?âøVCæ?ï÷q@ŠØ?øAÔ¶¦@J=g>¨‡¿ïùæÁ²À?ï}4ßݵ¿ëG¾Ûr'¿ÏkZXæ÷¿ÓkÁ¹É:¿é)g7F¾*UNASNone?ïOô-DäÙ?¥Bú»#3ö?`)%%¹¾?fæP½câ?"•2¾­"?¤ìöUÌë?ïV%ëàÑ3?£)˜Ù—ì?^Ì	oÆOh?ƒ¥'m®?"Nìétª?¡m¦gdמ?í*Úy³«U?›—rÙ
8?‡OºPI%q?~E«7Ø?³¿4èY€§?šåc|?îٓ˜Kf?›ÔwöÀîS?#"ô/V:?7Ãíü§[~?¢S2Šób?›ÏE7Z¹œ4FGL J0620.9+2201?¾¬úý°@/ !·"À:íFƒrèÀ<º&‰@$d/€ KÐ?ø÷3"«C?Ǽõ©ºÎó¿ŸÔ€Âªk?ÕQÓ1jÜ@Vô²ný¿ïÏJöžWn¿ÐÐM_Ú08?ïývþ«¿èÁ€}éºÄ¿Ì"O
TAÌ?±£až²UNASNone?ä~žþ7Î?Éê'fðÕä?Gì
Jñ´Î?Cæ‡*¾‰¢?ÖöÍ»^Š?ÉäϺù¾?àïé}DæH?Ж\¤äÆw?t<2O€0'?Šé鈊}?ÝÏ<<82°?ÐuôN–çw?çùOÙ¬Om?ªÖtír2­?"5ýŠ{)?t§Ç$?Î×`À§
?ª_óoç8>?析µÓ™Ÿ?»÷ÃÜüëu?Y™*j?`XS.<Àn?Ò©Ìû.ÌX?¼{TOä›4FGL J0622.5+3120?íV°ó
²@ K£ÂˆÀ:*3°1À;»©É'†@¦",0‹@žÜ~ñw§?Ñ`šŸ~
?妟Ԝ$@âZÛGº@ÉîvÚ?ïÛ·`Ô×?åå[¤k"³¿ã¸¥bûwÛ¿í͂iÒ+±¿î
^þ"¿ïý'AŽ?ÉUNASNone?ˊῊÓ?¾»d¬[/–?ÅÄ8߉ëŽ?Àôñ2)áj?ã¬o­¢h?Ƨó‡}É?ÅLYŽàù\?Ã\g¤¦òõ?Ûrü¢i6ø?Ë®üÿŽ?Ùæ֖&LZ?É<~a¶—?Õ¯Šy2•ÿ?«>sƒL?ÌÒX
¨"?¦­«:Âe?ÛçIy\ð?¬É˜]S3?ʙ–\nÅ?­(¿±nÎ?ߢWiðMh?»\žy›?ÓÝgØP?³i¦<*­4FGL J0624.7-4903?îؑԩ:!À8U»YÝÁèÀ:Õ}<kÁÀ<…´Eâb@òàY@@×Or.Å?Ð^Wú?ÔXsÉü7ô?þø_<¦y|?ÿÃVçmb¿âC"×ü¿Ü·ØIё¿ç›ÁýeñÌ¿çè"M×ú'¿ð?ïþª*
•…UNASNone?ï(…8pû?Ma"ùÿ¾?k߬Xj2Ý?jJôÕ9Ÿ´?—scfÓY4?œ8µèk	(?íâŠód‰=?ª±©Ìs¼7?…ÆYoom?'¨ñí‰F¦?¬eγ[T?¥Ýš×4¨?êf§#P™Ë?¥–z…¾¼–?«ÑNLL+š?"ü{rc?¾â¿Uß? §ùªÄ=?îD™Ðª´
?"†>k³ð?†´eï«Û?w{0•õ–?¦	I°Ôh?›‰Šn"4FGL J0625.5+7029?íy[bɛ6@7Y±ú¹o"À;ªçä€G¹À=µj°x@!jÄ@?ú±´"#˜?Ô;CMÄ?ÊI¢¶MÚS?õ‹Íþûô@‹=8ÌÛ¿ïÿâÙ~‹÷?ïÿúŒ—Ó¿èÞ*o¿yî葵†¿à]½Ž–[¿åª[Þ£
UNASNone?ïápº6O??iòÖ?x'ø?D4—þŽ ®??ùú$?w?i'Ê
86?h{fé…QÑ?ï'}€¦þ?Š"Ìáyk?I½þVOõ?Yv6rü?‰Ä¿ðàWÉ?‰%ȗ-{|?íärsÇ~?'p‡[ßÑL?ñaBu`?vœP5C?­<"+7yª?,O*Q?ïµcó³O?†mŽrâ?rN-›-$?iìi,ì–?™õȾM?…IÐÃÍn«4FGL J0631.0+5626¿©­A
D#1@3¥õß덂À;-DÏ<é•À<ÁŽêéîF@çÁÑ;?ÿúü‹z?ÑaæåQÓÝ?ӗ­µ°@Á[šZ‰¹?þ²Í‡²¼U¿ïàîzÔ]?ïF"y&²?̃K쓿Þ>˜â9›'¿é6Í0ŸÛ¿ïÿúŒ—ÓUNASNone?îñ½ªn¬‡?"»?u`?Š»-‰¬Õ?…©]MžÊ?"j³íTa?Üp5Ǭ®?íÛ·ƒÏ?«'шÇ?'¡'eŒ'Å?ž÷…î¬?©}‹U	Ÿ+?¢£ÜÉMŽŠ?ë˨¯©ù?¡ì5î>?¤ƒQì?S?'R&['?·aÔc/?™€¤V	ð?ì]"6å¸?ŸÿYÖ_n?§BnçåÍ?•(è|Kë?³ƒÛêÅ_W?•šÅär4FGL J0632.7+1215?Ú1{U¿X?÷¦Kç_À:
á'ï¤À;†}=B€®@"'Ñÿ;µ@&eÅV·?Ëc¬¢µÍ?Ô
"þLf@	"•á~4¹@ƒwçî¿»Tÿá¢ô¿Ïxbmοæn'¾-øŒ¿ågµñ¾ô¿ïÿþˆ0»Š¿Ì<Vžó UNASNone?ÀŠX'`?±Â×+¼Ú?·­D3æ?²Zu3‹œ?éGÁXë;?»Fï‹D?Ô&&Ð×,?̵÷^[Å?³L'ÍR:¯?´Àk¿¦š?ãŽZ²íM?ÍAðÁGÆ?͕È>/í?¨»Y¢[Y?Â̲ï¸%?¡o0FÔ<?ãça4‹ªÅ?­ëpý¾°ú?Ø2´°¥@ÿ?­Aç˜6Q§?¼ÏhÅAH?›§óDƒ!?àL¸-˜?°œIó4FGL J0633.9+5840?ì;™)mj@4¾™A…ŽÀ;dûHábÀ<Õ±·Ÿ@ 	ËÚŸŒ@ÎÓš3ó?ŧ`Ÿý·?À­ëÇJ?ÂQœÀ? ª@ñ,}ŒrÀ?ïÈW¢~D©¿àW@Žeˆñ¿ä t´Ý¾¿á I·6ì¿ß‰ˆª^ü¿Ô´4iq3UNASNone?ïj€1+Õå?‡QÎ&Û9ï?Xï¦gÌó®?PÈñ™ßð6?' ÿtt?†gïÞö</?îÖß["Ž7?œÐ©SÌVè?ašöK:É?mñ÷ )?¡xZâþHÑ?›ZItT?íøÌâq0
?'¥eð³·?y4rA
çµ?gP3Εm?­L£Ë¢+?G(+
d'?î–N÷¦n??‰2'çt?w,Ȩçüñ?fBïÒùG¡?£µwp|Z?‰7ƒG£"Y4FGL J0634.6-3046c?é¨"EÐÝÀ0Ï8£µ|NÀ:8WšÀ<DOúêŠ@¶Ñ"@ÈòZ%"?ÃyR¼»\¸?׏=Ë·?õ#ºð+w@qµ_ðý¿¾²»(µ€Ö¿å«;þ/¿ì¥• æ"õ¿àê¢Àß®§¿ê˾ßK¿ïÿøÞ£ŽæUNASNone ?ïÈs'†?–.ø{Q?,ý˛Ìù?-5©i°?ŠtKþ"}?ˆ7ž´Ü4D?8Íq?ž¦e èëç?n8‹öj[Q?"µFE?˜§˜Za?™ánî\Ô¾?ìOHËû^q?Ÿâé³L•?–‹^ßÿ
Ó?‡ˆcßÁæ?·âáè%IÉ?›+ƒ²'a?îÜ;N1^:?†ï©›qÞ?Œ f3X;?{Éúîÿrq?–(c (4?ƒ×+}>ã4FGL J0640.9-5204¿ì]9ů³HÀ6Ÿ(ǟfbÀ;Ì
V)ØAÀ<ê?ÉC«P@ Éí
4?þáÁçâÓ?ÛÚ-þ•ò›?²ÞÐZuíB?ÚÂÑ84$@	Î{"¶
¿ïü3ŒõFi?ïþ^‡tÔ¿çQ°''¾¿â?bžÍ¶¿V"ì"q¿ðUNASNone?ïæʎ@ê«?é‡ŒÆJ1?!¯7´'?9Df©aO?hfË£i¤?«TÚi+?﨧®h8Ã?'1
²«?4"¯Äƒe?Z
òAhõ?…53Ps«?'š˜×mË[?í·A	s»±?Ÿ"¤ÒP`M?fIqѓiá?h%oÅV?±"¬%Շ%?ŸWìÎ_Fx?ï²23›PH?s.j¬
¯?QÃÌ€ñ?P\dÊc4?ƒDϑ"á%?s4V$ëê4FGL J0642.4+1048?Õÿ…)R½E@{XÑRm‹À9ïL}‡\À;'Z5Ö{¢@‡åÇÅ{ö@F¿Ä§?ɐ]b²?ÖIí{ì
@>)#øÁ@TbCÁö°?ïä©B."Ó¿ßÄøÂôܶ¿é¼O§@¿çòáԛÎ'¿ïÿùSt?ïø#ÝÕ³¦UNASNone?è±.¶V—?¾üˆM£mÐ?'§Çx]Ý?	´ýrb?ËP-¶–B?½Ü#ó¤?âËÒ¥*õ?Ч‰Àáó"?§û Üd?³¼2§uhÕ?׈YÖ5ùw?Ï-6éAá*?âז«±nS?²ÿÀ‡Õå?²°4~÷e?—Kƒrʜr?Õ¤ÎÛ}e€?±x>eÊ"?åÓÛÈM¯ð?³OòõI(ì?£.æq;)¾?ŒÄRçŒHÙ?Ñòk¡=:é?²Ã*('!,4FGL J0642.9-6501?Ì"1°Hª
À9L[9âyÝÀ:‹¾‰=+À<gñx7@qGÛ
þ@¬ÂPr[?È«k=»¢X?²6ÊA'+i?ãEºßd@Ù¢.¾"`¿àûs¾¾—*¿âº›aÅ¿çvx݌b¤¿ã'eMa²¢¿ïÿ¾&@Üi?Á#%^‰MFUNASNone?ï^¢zž?'^6	3ë?b^Ì
?Yº	1M‡n?'ë¢G×*¿?ØF–nè…?ï8Á¬Û"I?"c×=ƒ?Vû@Çi"T?e÷wÓÂÅ?—xXäË?'ñNþÛ$5?íÝ»Ìý;?'ê"î?'ÌL%uΜ?sìH¿]d?­q;¹Ò¸¦?nŠ2€Ì?ï4)å?€k"ìŠF?r+ÀH'òt?`Z\‹"?˜ÔM'Zº?~Ƶá²4FGL J0648.6-3623?ã%'ƒLÀ07jøœ^pÀ:ÐrûÀ<A5" ¼8@û˜‰y:ÿ@ù—"ÆÔe?ÕGwB¬¢á?Ö~<ЕÚ@Þò"z–@%xÄ¥?ïgF€l÷пã"E	Œ³¿å/Gì'Ü¿ê;ÔÂd"¿á—½¡`¸R¿ïÿþó…õUNASNone?ìك{† §?±mD'eî?†Ã.3<'?†¹ÄVpšÙ?¶[~]cué?°tOOrV?îPºN";?§ßÚї½?€
[b|1S?*,»×•"?¦ñÀRw¿ö?¤G}/iOr?é¡ÿzt?¨<M©Ì?­Ou6Àb«?"·Ê›džf?Â'ºfQý†?¢ZÏÚÈ?í(h]¬‰Ö?•B³þï\ç?€ªÀýKŗ?rÿ]œèÁ?´§dòò8?"Bê–Y"z4FGL J0650.2-5144¿ê±4ÝF0€À5'	"ãÿïÀ:â$GÝå#À<ž¡ü>ª`@!N
©§-×?øñ¤óið?ҋ‹#ŠÑ?Í5Táä·?û±¾‰=+@†+ëÁ.´?ïúöv'"¿íx¾W¿¿×ÉA|¢¿×Û;Û"zÿ¿Ý;ƒ"…F¿Øƪß<;UNASNone?öð'? ©cÑfê?fQqn!?]ßw;ŒQÄ?¦™Ià? A‰(#ُ?î"Ð?ÿD?¤FÕòb1R?o3¦Ôª?{t;nÙ[?¥¿ËE"Á)?£KXq=rô?í4q§Ç?—×'J?{îs"áT?n²tÂt?´(ýô?–¤£ò3ËÞ?é3ʍð/î?¦pRià?z%:??p½iÏ3?Ê_¬ëƦy?¦•æ˜rÁ4FGL J0651.9-4330¿ÐZü$ÿÀ24GñQçÀ:Ò¢ªºSNÀ<K Ÿ²¸@¶å‹Š7@jUp
?ÖĶv$J?â³7É
û?ýDr‹7×@
M"¿ä|m¾I|¿Ñ!åBq£¿è%–ýÝæÑ¿ïö¶?¯?îœÏä¯A¢¿Ëg!!bÑ1UNASNone?ï§l‹ß?c˜2o²r?è"{ah?ƒ@î<sÊ ?–w
,0Óz?˜Œµ¡¸ž?î2?ntü?µCp"¦.?‡DàPPl(?ž:€û<?§
Ñ«¥B?±hµÿÎ?éØJ—ch¥?¨m]ò_?­Iç2¶Ý?•Àd•jȆ?ÁL[Õí/¶?£rtNÖB˜?îì;`›Ñ?˜Ô¼ßOÐå?J²1ñˆ^Ï?UOw? Ñ…ò0!†?˜Œs‰×7u4FGL J0652.8-1855¿è>ö«¡±À jÑÐAÌSÀ:¤V¦ÖÀ;¬ƒ•KV@@™vÈß,v@±«Vç?Î3[!8ßÅ?ÇFM^;J?÷b¢Œ‡b_@¯ãËh?ïÛ †ó¥¿äÒ¬9¯N¿äÕK@ÆÔ¿êäÞבL¿ïó¾ýq?•¦í}XUNASNone?á¹Ô€³?ρklΦ?ˆ}-¥_?‰Î¬‰*)?ÛÈnmÖã ?ÃmßRDlN?Ú­Þ?»Z?ÉwƒËq?‹Z2ÖÁ??$ÖRm?â$¶*Н?ɋ*?áš"®?°2aж??³<e(ddJ?—=¾–Üžq?×üÂpŠ°Ç?­[¾Ø`?ãóLÔƒ)?®à§«Î[ï? ‡n<)V?‡&»*!æ?Öxa×%?®kÇ}&†4FGL J0654.0-4658?äp,·²Î
À3
#Ä*fÜÀ;ja©ÊÀ<Y­}|,¡@yåŸ+ª@ù7ªÉm?Ãr(üÎr>¿±€ð«NLê?íçAÃîä@ƒÃvŒÏ1?íVþ–¶¿êŽ|/%‡¿×Jä•@n…¿ìg«ud0+?½ÍË`¢=h¿âŽ9žÝ%`UNASNone?î9~/
ô?¦†§nòžW?r85¯;?p"	Ò£?ª!(©Ùf?¥È%‰$?îéõùbÝ?¥‹8Ž€K?d‰ý؇]?{ÿk±ò_? % ÂèÙ»?£Ð\7ÆJ?ìê"q=‹}?š@¶‹f[†?‡P1•Eþ?€4{(Cî?µÁÖTû\?—µCxásÇ?í99lƒœ7? ®Û¾ ¦-?^²Ôê["Í?^Õd?©?µ»iH9¯í? ‹|ölb4FGL J0656.5+4218¿·¦äw6¸ç@2ÄÓ¿/UXÀ:û
ìQÍRÀ<~܏¸oH@ êÝïßÌ?ýÚy°Æ?ˑ<ÓÅåR?Ƙf?Ïú?üvÕIs™@€ž'&ޑ?痢–'R¿à'ƁY0ô¿³ðýmZ¿Ú7Ûu¼Æ¿æšaÙ¿Ï×æ'öÀUNASNone?íó"Iȍ? 
;³"À?tO#»S­›?j—vQZ‡Æ?®<æì
'o?ŸɸzÐ?íQ¥&>¾w?°Z'µ†s?…""iòš?‹±Å3­ú?²Î†@ÖMð?®"
c2?ígWƎd?•`
çŽT?€E]Áï²?pô\j—¾?±|$–NÝ?"}.è–?藚l¥É_?¤—'EJ'?šÊD±(sÄ?…\2â+Ü@?ÊHM·CÌ?¤[»o¹è4FGL J0657.4-4658?é‰}†'TÀ2'¶|(o‹À:ÈÈðŸ:À<›7W…"@Ý)ÆøÍ\?ýËj|uœd?Ì<>Y'?ß<Öàvø°@
¿Þd¤ÅG@Ia}žf]?éù¹à?Óë{#6æÇ¿Ø«€ÁF¿àå½^šÀ¿ïþ°_-âç¿è1ö½aÿUNASNone3FGL J0657.6-4701?éîOE;Ã^?ºG,k0ä=?Ã`^Q÷?¹N"yb?£š¢3ö';?˜äž»–Mô?åZ2Ê$×?Æ%ˆhâB¿?È:1^Â?Äùc'?Á"eÖN‡?´ô,D)–õ?ã6'H"?³S­èÿ8?ÌìьÍñ3?°'¢fÐé?Æ8éR©'‹?¥aTÿòCÊ?ä!˜咼?¬ª­sçÜ)?ʑS$w/º?­ÐI¨?ÄèLcò…R? 7Åc"†4FGL J0658.7+2318¿à9Ò	Þ·A@'Ñ"D¿À:Ï-˜¿À<eÅööq@&=Kþ@غ@Ù$?¸5%¦­©¿'µÜïB?·/ù‰@ѾÎ]?îÝ)4­¿àø»Ó€E5¿çË¿m"¬¿äsšA	_¥¿ãbá@øÔ¿Ò&c«KžUNASNone3FGL J0658.8+2318?íegô!AV?­@CvlÕ?hùZÖ
¼?_AêQWV¬?´÷¼D÷?¬àV:β??í3Ôç™?¹†u9´Æ"?fv	ì3]m?|9€ÁšN?µ­¯ˆ(U?¹!º'¨L?ìΛÒö"m?ŸE\n§êB?…æÿ0Ñ°K?s¬}V*A5?¶ÎA'1.?œ²®\–l?î©áÏ"õ?€˜CP+@6?mwåŽð ?V㾂ÒV?£Šv­Ñ²?€&CRôîI4FGL J0700.2-5118¿éI×SRQÀ3‰æÿ}úÀ:ü`8NûçÀ< !¥l5³@—€Ã^äè@óû¶Å$?ÈW2ÁÉ8™?ºäù}º–?ð] ½é¨?õs˜Ôw¼?ïû¿ß(™ý¿àCòÖKҿҁ~ƒ=¸¿äÐeÁ•a¿ïÝUE¬²{?îíŽ]ü4™UNASNone?若@F–?˜àð1Õˆ?`†Ì¢{ÊÌ?]¯¨C͉K?ššo㧳ù?˜?‹8ùC?ìùÞÅ­Û?¶»ßýB›"?'©‹Óbu?žVÙÌ(:
?³†Ã/¢À‹?³C¸Ôl;€?ìÕÞ랁?›I2¸»¢k?˜U~
Z×?ŒÞéB'¾I?³;©"ÿµ??"~öi¥Í?çßò¥Hò'?«Ÿp£è™|?ª1¶sEßÙ?™;€j|fž?ÉóÇÎ
¾?©'ðÜãµ4FGL J0700.4-4308¿ÞVœ€À0¤a¶Ô=À:ž;¼n°¸À<AäMòÒ@ý¦kd@8—Ü*7â?ÄÆFuÛ#}?™|cÓ¹ü?ÐԁLá@©zJP?×,B®{S¿åV«€'¿îÆ!·à¬¿¢	_$RÅ ¿ïÿÿ" 5•?ïó@oܲUNASNone?ï‰véÒ ª?ŒªßñhPM?lÜÏ+½s?iú¡ÿ	¹?†kÀhxÏ?‰.N.òc?ïnBYå‹?"?Y'é ?XÿÚ­ ây?wÕIh´ôº?¬Ú	é@‡?'IÌàò¥?í'Ôóæcd?š†wï¶?…RR0Ž?vˆÕŽ
ü?´ ΆáÕ?™ä;Íñ?ï_ÃE!¬å?"`Wµ,?jq1-{¨?e%Øänñã?ÄI5¤³ï?'–¢133Ú4FGL J0700.6+3558?鍛'Ž@1Cð#éêÀ:¾í¥Šh¤À<…˜f"³@þBƒ2O?ÿ'
;Qå¦?ËB%ŠÌ?Ø#ïÞʦ,@
9'N"¢Â?ýNÀ'"ß?ì'JSá)¿Ðè=µ¿ÜÞÝÛèɃ¿å¬•õ *­¿í`Ÿb0vÀ¿ïþ~á•›UNASNone3FGL J0700.6+3557?à0í²gʎ?ÂM¯¯ǹ?Àdú£cµ?µ‡M`lQ?×l Þ¹
?Áö6lQ	+?äRÐ4"'Ó?ÆÒõË·fp?Å	³˜Vúò?ÀþwQXîÓ?É«•–½Ã?Ài³EÛÚ?ä"¦?é?°(px‡]ì?Å<Џk+'?§Ó>:û¹?Ȳ¸×˜¤Ú?¥ÔìrñÜ?ä7Í$0á?§éOoåæ?Ãrº—róW?¢ÉùW­þ?˯3üI#?¢£v»ðGê4FGL J0700.8+1551?Ð<Ó­3 á@"^ËtÝønÀ:ÕZ±&~À<u˕•(@›Ãl{Ô7?û6KÄúp?ÓoI#Šs·?ܪù=n˜@Õe!ÂÈg?ýiÀÆY@8?ïøc‰<TD¿Õ×u1ÛD_¿£âï#
÷¿Ümz÷÷ž¿èƒÜ=®l¿ïÿËÝcßUNASNone?äÒ琡f?¯w"'¸?›,ߪ^˜?•F¿Ð?Ô§oÀî?Âët¶¥†?Óíä¡æÕ?ÆOƒ:3Ì­?­`ƒC¦ød?¯ÖÍÿØøð?ä3zҌ?Åùk›•¬?èIRGï?§Üaï×þÙ?©Ä˜øLÛö?'©>1ä²
?Èi¥ŒI?£ÉC_B×?ã¾E²H{?¨7ž³ýìo?²¦"¶A?šã¶»Vj?ÓÙÏmíbª?§¼WqNšµ4FGL J0701.3-0403¿ã셾½P?ÕÏæݚ$"À9dYbqå À;BöÜjς@aR½è@Rr†/YŠ?Æ-¡º$?Ͳt†åŒâ@%ÏÅ¥'?ûPü#ý`>?îèŒEô?Ð)ú¥M,¿ênar
ßW¿è"»ìª¸¦¿ïý ‡_r¿àÕ,ß?–UNASNone?ÍfÓ³?À.¹pé?«ˆWÄd®?ª7óGðiƒ?ç6*È^?Á4»Ñ ?Áãè}b?Á«'×6Ë?Á"I«?ÁÀ¡šBv??ç@àæšeò?ÉOð	¬óÚ?Ґ7@åM?®ÐÕ
A?½ómHîÛº?›¹£ÑQ–Œ?âùv¶ožb?¯!õ¯Å?ÉWm°^õŸ?¤g¿ÈTÌ?ЩFÚ¦T?±™'â7?áU›ðzïo?µ^›ýX_4FGL J0701.5-2842?Ü¢;6@YÀ%GOøe×ËÀ:ûІ•°×À<CgUy¯@lþáòο@Y™~Á¦ÿ?É<Õ"oß¿›'Z¹gž?Òo_Éî@×~I1!`?ïݬþüõ?£`,¡¯ÎË¿ê§ýuDØ¿âTÁ"tŸ¿Ò‰À¾Kª£¿âª†7"ëUNASNone?áêOTI"?Æ¢/WÞ(?rðA/òx+?jQÁÒ°9?Ûà0\—¢÷?Ɯªï~?êu¬ˆ¬­š?ÂÚ؉l?TL_õ¼Ô?gKÓÚöÁ?ƵcF?¾¸ÊŒ#?ê¢OyZKo?¤F4(S²8?æKz9Í?w Ç&W¨?Ã¥Cµß.¨?¢ÒPçÙú4?îw4ÂbPå?ŠON''?]'àÔªtj?R«³Ú¹ð?§ Ó5ž?‰ÉÀzzÒ4FGL J0704.3-4829?Ô orZÀ1ô$¢v·íÀ:º¶â¼yÀ<V "oeé@ ]¾!8_?ÿoÕ`EK?Ìvô©	Ï?¶vS€ÕS?ìki¥¶Ž@ëuró½|¿ïñ±ôr{?ï÷á]¨|¶¿çi2(q8R¿Ò±K¼ìÚß¿åžbP2¿ådi×4.ÜUNASNone3FGL J0704.3-4828?ï½ji»^?u2é;3…?5"ƒÁZv\?/ó½¿|cL?ò'æ;V¾?t ?ï¹P»­	?"†
Ûo$?1H—}â°?D7rÀ°¯£?Xθ?ƒ˜¿'?î_ÍQ~ñ¸?öÓ^ß?iªaõš?V•*¾Õæ?¨hˆòe-?Ž¨üBD0g?îºb¿4€?"'@×,ßW?l¤T*?\dÎS~9p?¢ŽÌªöw?" h¨Î4FGL J0705.8-0004?á$÷ä±#@	\[cÓåÀ:"Ö¼À;¾7¹ª±@¥pŠí@¹÷<âß^?ÊàÓnu)?ÕYâµí7@ñžBuÆ?ü¹¼yÃep?²Áýäê%?ï\ÂMÂÖ¿âQ%!!¸·¿éè¢ì(²§¿ïì7Ì'ã?îi,êCÖUNASNone3FGL J0705.7-0006?ÔZšÙß?ÂÚÕóX}A?Ã9;_N*ô?º%]üW?á**úßS?Äê-ÆIL?Í+ؘ<žþ?ÇFbÓ!?Î÷«\ö•]?Æ91b"˜÷?à÷³2é?ËǬ Œb?ԃÓRѼÉ?ªùkbØ*?ÈQö¶¾?£Ê"À!?ßS1^¢çØ?¬Š#šÑú°?יèµi~?°Ñ?FZ¯í?Óp9
Tî?µ£úœÐåŽ?ÔõÞ9‰"?°ò¢aßÚ´4FGL J0708.6+1747¿äÎy…eý@'k͚R&>À:íÚü:x¢À<c;8»2@ ‹34à²]?þ{®—WŸú?Ð6[œ2ü?¶2ðÞ¤æ?ꖉ1+?ÿB¥Áðü¿îÉÔž›·?ïý¨6ëN˜¿å-ë?ÿtj¿àȖg"N¿×R[ø#h¿åû®Í…/UNASNone3FGL J0708.7+1747?íçbº¯óQ?¨+^Æ|ÿ"?Têt½Ú=?OÉ	âW?°q@ZAn?¨MÜþy?í•f1Exƒ?´+À‰Ýï<?d÷ãCÕÅ?qÞd#Ü?²­Nº5?³ãHð"8,?ìÒk¾–IL?Ÿ_)gïñ|? 82ÁþL?lë&‰P'?·zžˆ!•·?À£9±?ìÎásǃD?–5''\É?à¶¤?s•|ó8Î%?·hX^Í+?–pÁó«Ø4FGL J0709.1-1034c¿Ñjfõœ=¨¿íKÒ»úÀ9!ÌzdJÀ;1œ_F·t@üx±—'-@ÁåGíÕ? y‡«ZŒ?ÓÊ89W@¦ÜG©ã?þ0n&nª¿É¢ãj_D¿ÞÒý¾\G¿èQÒ?ÓT¦¿é°‡ÿ=¿ëoc/zA¿ïý…1,ȶUNASNone$?³²zǂüN?¥/Åm?Íんž?À8øÓÉ`Ò?æH7Æj¸ï?ÂÕ:Q´?¦Ç^8=÷?¤'ež:Ñ?Í^‹² /?ÃÖó¦¦Yµ?çG`"vT?ÃömÃ/‰â?Å´¦6lBo?¤	qrR?Í£x¾é?« éÄSè?ã*55!?°_I×?§–%þúØ|?‡ ëcþLã?Ûç$aܟy?±vÄy²³?à"o"¼?±:Ä,C¨4FGL J0712.0-6431?Þ Ì‰!ÓÀ6*¦óõ/ÂÀ;'24/²uÀ=ï4Ö¡b@§!,JŒ?ý8ø¤ÁëÈ?ÑUØInß?çï~U@Jâ|az?ùÜ÷&èw"¿îªi?ߓú?Ó߁w^¿È*è7¿ãÆ}'s¿ïÿ¤Á	?¨~¡½÷¿6UNASNone3FGL J0712.2-6436?à£JIVñ,?ÅÅÅ.ÛV§?ÖÞ4ÐBn?Æ΄>·Õ=?¿lÚt>¼f?µ‡qF$¨Ì?Õä;Qœ½)?Êc†6½?߀úð/¸?Í¡`UÔsÜ?IJ‡fæ&;?ºa.XÄ$Z?Ó[·fµß?¶\F³¹{E?à³ýíiaº?¹@úå¦r?Æx™|î»	?¦g–æ(	?ßFlàþì?´›"E‹&?×mҕÏç?µ7	ÙXŠ?˜+úž3ò?£ô	žŒiB4FGL J0712.8-5637¿íöÔBëj¥À3"µþT.UÀ:¢P0™û¿À<bg.'Å@ôê†ñ÷)@"dUêî ?ËHhbj?Öq"'›@x—Ü*7â?ÿ5Œu?æâ"Ÿg9¿Â'N¹Ìiû¿èϕÔèû¿ëf YžØ¿Û<-'ÅË¿ïþæZ<ŒxUNASNone?ìÜNóLÇ?³5j3?—?4ó[ð?–¶BHFðJ?¹IPKŽ¹Ï?°ÿÊÒLî?ëôÆóeì…?¸B"r«Ëy?¢/¥"‡¼?¨"÷TËÇ?·Aõ›Óv?²NdußQ?éFQ–'?§bƒ½×?°ÈLtDø€?™ACF‡x?ÁfÁŒ—+%?¡]Ëì#6?èe£r<@f?¥WùÖ@q?°ùSÜp‰?œî+/¤ÄÏ?Æ_õ Æ#?¡‰¡|¡M4FGL J0713.5-2555?ﱶmÀ Â	$lÀ:`öqÀ;ôó±³l@"®R
hô@éu½~â?ÂC| 7?•g'ߐô¯?ÖÑá^ª/i?ý¼&1$4?ïa‹€|<<¿Þà¾FL@¿è´÷Ãñ[ø¿èû9Ç¡ë¿Ð±©ûçl‹¿æD˜5kUNASNone?åòïBvÃ?¿ì®þÄùX?'¼¼šôØq?wuÀäcõŠ?ӄ;–ék¸?¿ÈD9ˆöW?àüAzÛ©ü?ǼdÙO½h?i¤Ï"ÂDƒ?zyÆûÂâ?ÝÔ3l'~?ǧ"wЎ"?æ)ä ¬¥i?®ƒÀWÿ?ŸsgÑ'¶?ƒ¥"/«
à?ѵNi¢²?¬'}ŠŽª³?êìã‰÷H°?¢;˜F¯î?…({'ÓÎ?w/¿Îw¸[?Âùñ i°?¡—``Ÿñ4FGL J0713.8-4820c¿Âé@µ#tÀ0q+àŠðÀ:Ä©°ãÀ<G#çÆM@«<Û}"«@âÑk—þ?ÉâxÉhi?™OSǟ³±?Ñ&±dç`L?ý¨Tßd¿ÖX‹ýy½Ü¿ãCÿ~zÚ<¿ékEÞ±{¹¿Ûý¥|üªá¿êöÁBU&¿ïþ:bÒ]0UNASNone ?î'Á,»W?œ—Ž 8?sðò½sÒj?jŽ¾ú~Ǖ?¤eÎܜƒ?›+6f]…j?ïÍ(ÁB?›'èj?[×þÀ=Fø?jÐd³F?›hÛäp?š@^;?$ê?íä *VÜ?–"ZpùÈ?…Õ/CÒÓ?wO×+#.?±652îº?"Åî›Õc¨?í9Í­ÉB?'íC†€™?ÍrŒà-Á?kÚ|ÓðW?±¼ƒ@õ°=?'û\{¤4FGL J0715.7-1128?î˜I,;>½?´ÿ¾'ÜÈÀ9¼÷~0ˆÀ;`Πâc7@o!c'Å@¢Ž…i`í?Î7^¦~"j?Ú°km6d@@º°k?ꏳ`Xôþ¿Ü*«Ú佄¿¹ž+࿯¿èðCÊZ+Æ¿êN›n…êLžsóí£¿ç+ áCUNASNone?Ç
NGBáú?Ä3n*Ü?´BÞ^¯d?³|A<àÍ?çµ¢Ye5?ŃZJgÔ?¯à˜®¸Ü‰?µ–_Üu|Ê?ÈkÐ[´wº?ÅùæL.&?çç^'TI?Æ|±âÇC?È:d<CÞj?¥QžVìB?Â"24y?ŸÖ-žj•0?åmdb?ªº½Ž?¦ýf<t/s?‰â͹‹Ñ%?ݳo¨[Z?µélCbï–?ßläɸ?µÉ«ª"14FGL J0716.0-0826¿ïQ'bñðP?ù<¼~ ïÏÀ:$OTÑélÀ;¬ÓW*‰A@ç|\@?"Àh¡?Ð(Zý|˜?Ô)ù"Á ?ùb.þñG?ñrZ5*¯+?´Äúâ‰Í¿Óãº¥¿èq'>3Av¿é¢á ÁÁ¿ïøìˆ3@?ïÂpóˆ"yUNASNone?äÖçS1é?ÅÉú…i{?¢­ñ¦,ÚÉ?¤¦$%6rb?Óþ=ü"Ó?ÅOóN*cP?ÏÌuPm3¸?̤/™‰)1?¾/6áø'ñ?šrF"ÂÒ?äFûÏ¥®?Ï2nBë}&?׬"--‹?¬hù÷`?ÂÄN·åÛ? ŸÌåŒËá?ÞñT°ö߈?¬jÇÙ!æª?ÈémµßüÍ?ªqð{?ʺò³I x?°ëÂõ´Î>?ãç嵸®?³`ÿm%¤4FGL J0718.8-5004¿êï{¯½Œ,À0Z\å´$_À:͇
JܝÀ<…f?Ð@³â@0Ö­3ª?Ëq}Ü#×Ì?Ú~FïƒÜ@¬>/æx@ ¸=s¨ï?ï›ÞÒê¿ÒOZ±&~¿ÜŽèÑQ­¿äÞ!ž`RÑ¿éO"¡2O¿ðUNASNone3FGL J0718.9-5004?ç"ʤ‡)n?½ð1úÞºŸ?½rwg%N?³œ{xÉj{?Ä»™ä/Ǥ?µ»‰c¤?è—Âë±ð3?Â#ÅÎc˜?¸–ÊŸ-€Z?·Ø¥Èÿg°?ÁU¡?¹¨}|(	×?å;""Ö=?±ÂôÉTéÏ?ÆÚy!í
0?«¾ŠÓuWþ?Ř˿™Õ?¤´¿OI?ἀð-×o?§«x£,Æó?Á'b?¢O—ÎÕå?ÓÀjndÅ?¤°Ìá4FGL J0722.4-2650?³\Üp¸À¬	Þ¦%À:ƒsñidHÀ<D)ÿ®@\ó4ëo$?ÿ:¤þQª?Ð=;"G?á%K~ƒ"ž@aL¾´?þšBѶÁs¿ëqA@'m¿Ú‹2äôQ¿Ï4`¯Ã'¿åËDÂ&ք¿ïý¨¢K?¦«Qý΢eUNASNone3FGL J0722.2-2648?ÏeX§¦¿?½gj
<þ?»\eú©0/?²ÓtDŽ?ä»9€ðK?Á'¨Ô{H"?ÌDB×·¥¤?ÃhÔö8jF?¬™¤Ÿ]‡¾?±ã9-'&L?ç%U>?ĊIsð?Û ¤¦uÏ?°íːÚbà?Ìc¬–.i?«ÁF:"Ð?Ö-…sÝý?­½›¢ëÙ?áF &%ä?°ƒ†d#?¼3Ÿ£ñ+H?¢¯ä@K?Öe×ʹd?­ƒƒ`Ã
w4FGL J0722.7-2309c¿ÆëBS]öÀ:og—À9šñÎäÕÀ;LzÜ?0—@Cÿ‰7¢@y͛ÿ¥g?Ê»y'¾?ÓE‡~d	@	êºp©¶?üXùÁL'?Uª×¿å3éèwM¿èՉÕwõ¿ì;C½Äò
¿ð?ðUNASNone ?â"þ¨7w?Ņ,š{ÿ?¬›ˆõ9d?©õ¼çÁ?×F>rj¬?ÄÿñÈÕ
—?ɾ»‡Ò®R?Å®W—žN?¶nµ»œP?¹š–ãpðí?æÂz|óàá?Çì"Ba'?ԋ`MÞ/?°Æb
 ˜?À»½¸Ì­ç? …±û¶?á‹`k@eo?°ãòªTk?´˳m~Ö?¤Bæ)úLt?̍÷×£Ë`?°pæçë?ä/O;­s?±¸»½‰¼B4FGL J0723.1-3048?ØY=iÔRÀp®SeâÀ:¬ä_‰PÀ<<v`¯m@@ÅIìˆ)@NŽ£œQÛ?À÷5Á'쯿˜šŸ˜·?Ü´O'…€?÷Q•"&h?î"gñ€á<¿ç[}Õ¿å÷ù1~'¿çŒþ«—¿Ú¡ûÁVÍ¿³+ooyŠ…UNASNone?äûã!'J??ÀªŒsð	?x‹05>h¤?nFð‹™hG?Õ¦üqÝ?À_–Ѝ?ÙIû^ý?ř0'«þÎ?t0ޟ Ì?".d/Œ5…?ã38CP?ō|è?èçi$¾ë?¥Öx–å…?'&ÑqÁrã?uÏùɅ1h?Ê=>Ì%u?¤Åf.S
õ?çPV‡´?¨ëòûáS?"؛M¹œ?…ZFG:†?Кò9žþ?©['\Ç]"4FGL J0724.8+3016?½æÍK@3öuy(àÊÀ;±™]3·½À<½`µL}‡@#nxY$È?ùÝ5µÄr‹?Ƕ÷xr¥¿¨ócå$?âEy¡¬'@šŽË·¿ïÿDÿ8"×?ïÿï0l¯¿æôpŸû2'¿Ñüf£".~¿ê•ïUÑ?áºæ ³iNUNASNone?ïáÊ-Ji?lž
óœÕ‹?30FKju?8'Lz°x?l-Œ(Û?kŽ€þx`?îátQï?±É;z¼?S«ŒiµOÈ?e…ÂÌÚw?¡QW"e)?±§Ýg"?íu@ó­û'?šÌ¦¨û?|¥3ûìµ$?t;Ø>#Y?²‹¥"Ñ[v?™ò›¹ð÷?ìïíÕcŸH?©‰â%»Tï?~¸Ü±íØo?E¸¾?¶•‰Ä(5?ª­Ú´ž 4FGL J0725.3-2550c?ã øBÇOàÀ†¤û¨'À9Íí'?2EÀ;c¡®;N@-8œ(À@Åôÿý²?æhàÿ‰¸{?äužö$à@
-«Þ7@È{"ZÃ?_î}!¿á¼üJÈü¿èÛrLM¶l¿ïün{Þ¿èÁÞ\AIv?хõB6Ü5UNASNone ?äµédµ|¢?Ⱦv.0§m?´"¿Y^?´79ë?ы}`=€¼?ÆHÉðFÎ?Ñ·ÎP–6¶?Ê?gð6$	?¹†|R'¤¾?½ÖVZ#i"?ãóIMb?Ë«žû?ÕáaÅøo?°71€æJf?ÃQøe̸?¦&áÿ¸æ?àN:»š?±_ª¼í?ÖÏ|³ñÊ{?¹«ªf®²?¹À'¶:*?¹ÚÓÏÉ?á`=Ó°S}?¿Ýa^¬ñ4FGL J0725.6-5008¿Ýô•Âä/"À.À'ÏR¹
À;/ìVÕÐÀ<"ՐÀ­@ ÃÉñ%F¶?ÞW> YQ?Þ%œSÞ$?ï‡ÁàŠ™Ì?ýC·zU0´@-'U°5½?éQS¿Å¨@?áµVÄ1ó˜¿ëh"ÞÒ2è¿Â2ÏJ«tã¿ÍGöµÿV¿ðUNASNone3FGL J0725.4-5007?î`}ÑX‡F?¢é|™)«?€ÆtÒÇ?z.Všž#z?¥ó±fVø?¢%´s¨|M?í%$ž-Þ?ƒo{nÓ?"­š¹y?œ8V½J7'?´A'\Ÿn~?Á¯78b8Ù?ìqˆ®òÞí?žÓÈƼ<ê?•tnC]ɘ?ˆ¼5úà9?·ž÷'–3?š7{
,]?è`רF?¿ñ©Õ²¬ô?vé™bÑ=R?ƒJ‡T?Ï0±±ŠÕ?ÀÂF"4FGL J0725.7-0549¿á`ґô@¼ŒÖ<¸À:$ÕϪ͟À<'¤ýzê'@ ·E¼wÀ?ü.;—…Ã#?Äãâ'§ä¶?Ã"?Zˆâ'@üäŒØ@s	¶Z?æÝÿŸ²ãB?í€FacGM?Öå±àHþ¿ÛOȶ«¿ÜìØ:¿¯¿äJè0-UNASNone3FGL J0725.7-0550?è»ÙÀx?¿ìéú6$?·'Ê{&s?v*XVC;?ΣT'ªFs?¿µ®V›&-?è2ýSÃ?ÅmÖ`nQ=?tíØfhÍM?%ü¨?ÌãÈÐ×j‹?Äêés¹&?éo"‰ß;?ªRì3‡=‰?
áüÔ§ì?vßy¯l?Èpÿ¼'8'?¨ºïÕÓ|?ì¬"-À¤?Ÿåƒ€ŽŒ?‹Û…?€T¬î~NÌ?·#¬Žøs?žJà&濙4FGL J0731.0+6607?å°¢Î@<ž"šVWûÀ;	µólÀ<°5ŽWF8@ß\>oQr@N˜™¿YG?Ï^ç–ýˆ?Ë
ïWúh?ûѽ¥è@$ÃÆ=ç?Õâø]I\??ì'©
Oå¿ß§ñ¶'!%¿àt`YÜë(¿ïÂXúìñ?ë6ElÛNUNASNone?ìFf"‹˜y?±´ã´îÊ'?§ô€zšu?¢9ãŸS^A?±Ò‹ž•o?ªØCq}.N?í…9åîëf?­3yxñ?"¶p$m?›Ä°Äש?­Ÿhÿ	ß?¤	¾·Ë¥g?ëatOf²j?¢â]SÜÖ?§U^ډÞ?"¨ôO¿?¹I®…æ??›@zAÂ?í›þ¼Îx?›ÎZkðï¸?§ýç^»§?•™çbëos?§¨Xµwq\?Žë‰c¿Z{4FGL J0731.5-1910c¿ÚÌ0X|¿È*VÀ¬'À9vf}ãZ®À;$(U{]@àšF<Ð@@sÀÁü?Ð`ÏM°Œû?Û¹1Å{@Ÿ€Á[ƒ@oå¤ßóÆ?´¬˜¿â·Í⠜¿éHL՛¨h¿ìÃ+c[¿ïè¶!å'ü?ï£êUsÐUNASNone3FGL J0731.7-1914c!?ƕ3˜Â??¾Úì±eî?°}2¿ãá?ªõvU¯©`?èKSw~t?ÁŸe©b@l?ÌVåͱê™?ÈsVaSà?±'ĞýH?³×\1'¢¡?æÅMø³ãq?ÉðÒÒ4YÕ?Ñnj±&ƒ?®za¿@[?Áq¨™þ?Ÿë¼õy?âÛvýF??°5±/ê¥?Ë=
{d6?°:0"Õm?»Û¨¦îښ?£©^I§'4?åµHLI#?´-h‰®b4FGL J0734.3-4448?ïìY~Ò=À'ƒÌòŒyöÀ;ÔÈ("À<bZ¬ôÀ1@ Z¥@ð@>GÜ7£Û?ÃÍí^<Ì9¿Ÿ\1%´;ÿ?ÝC]÷)?ÿÈ¥Ó¹¥ÿ¿¼ șڿá \a)惿éQÓÂ_`Ž¿ÞÀúôÓQ¿á]Õh|Á¿Ö…Ôàík(UNASNone?îf<Fú	?§¶ö𑠱?\Ès}?UÆ«•ÏŒP?¨¶+'ÂÑ?§l×oŽç?ëÙ09Ì?À*´Bg"t?\çg'.É?p¸YÏ?ÀapJ¼s®?Àú"Ê´?ìžqvpIå? ¦öŽ·ê?`ªïŽá®?nIe§mù?¹i"½?Ÿ|þš	WG?ìeñL? 	:7ûó?óä®Lø?qù…"ô?½؈½×? ;z¾_ûM4FGL J0736.9-3231¿ÅÆ…ß(ÀL™Â´EÀ9RyaíÎÀ;'¦éä4È@ˏ¼ÈÉ@$§š
\à?ºürùO7?ÕÒýhv@¦¢‹°£@—Ž§x*?ïÿñ_{'¿Ú;ô¢Ô«¾¿åÊZâN¿+¿ê÷']gå¿ïÿíPÐÓ?ïñÂjÉ"UNASNone3FGL J0737.2-3233?Ô°Ì
¯r?ÀÔԒ•'b?Ïäꂎ}ò?ÁI&mف#?Û\¾±	O?Âǐ"ñÑå?ÃwJiêï?Â@B®öe¡?Õ!^çWß?Ê1
5½Î?à'~¹õÕ?ÌXK"º…?ͨWèQ¾y?ª¾Íà"¯?ןSTÚZ?±¾Ðzý
Y?Ú+4¸'Fh?°"ºk'×?ÌÜY?ã´B?ªoƒ_N?ÖÁ,™?´³Í'?œ,?ۂµžá–H?³1\b/î4FGL J0737.4+6535?ïH«Ú'Ã@=@W:yx'À;TûwCÀ<Û:aû›@ Ÿï 3Ò@Ðh˜oÍî?¾¥õÝè(¿±Œ,ž™ˆ¨?ôn$ É8Ä@‡ó]ZN*?ïì³I¬¿ÒZž\!¿æø'}sHL¿á˜çBsB¿àØÏo>|=¿Öј
¨_/UNASNone?ïÜ¢¼Å†?nqZ%Mò±?A!&°Š?=*©t¹Î'?o90:œ?m—¡aìô?ï}=RÑÂ>?‰@1>Ujò?Jõö‰Û?YR@6KÌ=?[9¬?‡â&K™Ž?î¾ó瀀Õ?‹œ`´×¯f?f'õ,^Õ®?W2WBÝ>]?¢§'52N?‹\‰ÙØ?îν'œÞø? *'•çž?xF`v¤ñj?m8ݍ)"¸? [Ç]rV?œ{ž4FGL J0737.7-8047¿æ®îüˆ¸À8îÉâ6Á]À;mðwÌÀÀ<®rØœ@"E…sª?ûêՖŸê?˹®øP‰/? 33"'K?֓7_'·¨@–Æ4WK¿ïéZ¢
¢?ïödá+(£?êàöðŒÅv¿ßýS]?á¿ËA×e×ö!¿ä?y'"UNASNone?ïdWSH?®¹®Ç´*?0™³ýÍþ?(LŸ'ú?‹b0Ê<Â?®¹ÝÛäi?ï"Ý–øý?Žy¦Am¡S?:±1Xöj?UfZ	6øQ?‰ó05òÆ?OӎU+?íá³&3G ?'J"7‰m?k™ö»B?X!´¾²?°Éþ¯êô?'ˆà?îÌø©a1?ö*¸[?N?g ËÍ?N€|ˆš?¢·wÑ	ÑÃ?å¢ûñ£4FGL J0738.6+1311?ÛW5*#Á@0TC^úa[À:¡1¦¿óÀ<TÇ$íS@wð¶6y@È7 þ}I?ÀŸ9Q´~¿šÛ"CwÆ?Ô6߇Ï@¸¹jyN¿¥´)gØV¿éyô'ô;§¿ç)GŒ†‹ ¿ëËì't¹æ¿¹` Ò¿ç†lªMFUNASNone3FGL J0739.8+1312?ï0¥¶?•Ü³Ì.?nIÚ&‰‡?iÄÕvÜÅt?˜pÁFš·ö?"ÏÛFâ]?ïƒYñ²)?"VMF¸ä?Hù¤æߢú?a˜üÃ?šu%{ƒ?'"³"·Ì?îF˜Õ?7ÿ¥Ù7Æ?yƒŽU-?qUçe>¢?¨o"·xZ?ŽÂãõO?ï«zëÍI‡?oíÒ å'?@q?ž¶?9*bfål?"1Â=¥?o?¼ŸˆQ24FGL J0739.6-4530?áŸF]Ì'ÐÀ&~gµñ¾õÀ:€ÄK"À<ùqp…¤@üoò2b@ùI¥e·?Ж@.l?Ê"hܸ?û‹Jì\t?ð<x{í¿èIg–Øõ¿ßܔÀìĺ¿æ¢þ)q¿äç½~{0"¿ïÿ}ž¼C=¿ïÿ·¥ôïUNASNone?è<ü猸?¯çı©™?–q³IGQ±?¤…,2o?ÌAy£8âç?Áí—tþ€(?áÌ¿Ðfò‡?Ð×¾pà| ?¦ªïSµýá?­š©R<êï?ّ"t»[5?иµ."h?ç0÷xæ?­8©­ñ§?°o…{,?˜(O'øê?Ë_¶_^¨\?¨3·ðWñ+?á#ü'Ö¤%?³t¹¿ry?µ ÓÞyJ©?¡@Ýç,3?ØoÒ¸´e
?³'–ý<{4FGL J0741.0-5226?ٟ
Š{!<À,Xépq'#À;wï‡â·ñÀ<Œ¬&dØ@#E†•…ã¯?üCïÉQJ?Èùƒ<Ù¥¿±P;ל‰Ž?êÀSAÆsí@¸(Üî'¿ÌH…ªÏL¿ï-¸À%t"¿ÔM›iR¿ßWçÝõ>0¿åÃcÍ.ò\?´å€ÝNêUNASNone3FGL J0740.6-5230?ï—ÕjE?‡hg[Æ?1X5€ZbU?0nà¤Ð8?‰¯Hù{[Ù?†ªÕò?íâ¹B¥Ì?ÀVíuFû¯?[ߒmd|ø?y)·NêQ:?°z·¡!w¬?À<ʸHÄ?íÒâáÌ$?™ò°+Á‰?^wZZ·œ?TèRx:?°ïˆ4J€?™Ò.÷‡æp?ê—%Ò0?·Do´³q?eþ"{{/?i!'†U¡±?Ç1«'ÉS?·½6RC 4FGL J0743.2+4034¿ïmnK@:Yæ%cgÀ:ÎÓU}
À<~Güó@ÙJ¡!@|âąÖn?ʔ]Úü_?¸hšÉŽò?Ù‰@¢ŸÒå?íáH2ž¹¿ëzá³
Þæ¿î
# îø¿×,RÙÁ§Ö¿ïÿT©¥€X?ïÝe¡D‰UNASNone?ïÞ%Œ?pÍ®¾.$T?fðci?g¶'Pܙ?WÑÕ+é³
?`σçäf?î^Z)Wú?®wwÛ¬M3?†ÖC|_^¹? å!A16Ê?¤iù~R¨²?£ºóubc?í=\÷ag?–åHs< ç?ŠÕÂGƒ§ã?}k€î«?²º_üRß?"Ä"E2?ïw ´|,?ƒI°¢©¸t?{æFØ,ö?x®O0TT‡?"D¯'ðžˆ?y;׸'i4FGL J0744.4-1403?â^íð>Q@‹"ÞQZÀ:Qo­7PÀ;å‰bÙ@̀;¤›Ö@ÖwÁ½o?А^\¶#?×>š?‡@T¯ÕEAS?ôBñ—1Š?ï³ÃçJýT¿æÕ `]7é¿éº øžï¿ëÇC‹p+¿ã%áæåR¿ïÿÕ¾
iUNASNone?åá^>QŽ¥?ÃËд¨ƒf?±£–µÏV#?²¼'g¼È?Ϩ»«Ò]?Âl•z'?Ð*Í̳b4?ÅÐ1yÑ)?ÀçAÆ¥?¿Çìœßb?ãÃSŸÕÝ=?ÇÃ:ßõ'?à'^¥åþ?°H!aÇ]l?¿³<ÍJÕî?¢(þ:"J?Öîs'~ˆ?­*±‡ß?ÖÛ:Ϊ®Ÿ?¬¼Š` Ä?ÌeJGEç?²[Úð¦A?Úò 
Ô.m?°~9‹Âœ4FGL J0744.9-4028¿ï×җ"WÀþô›»³À:mµWeA£À<f
w"@š—ƒê°¸?ü˺bfý?ɪ`;Tþ?ãÄZ7ƒúÌ@ßbц@X—²Ž³?ïz͑êØ¿Òê?yg ?ÂâÙ(¦¿äÆhÏÍ2M¿ëFz£4M¿àƒ ˆ÷
UNASNone3FGL J0744.8-4028?ªùîå©?¢»ü\}P?Û@¡Ÿ·BR?ÅñuÜØ5q?à°?Õp}?ÅÙVî+¬á?ÈOÚPwð?Ä@ÄU]Ï?Ë.YLR¦?NJ¾šPLÇ?ã s+×Z›?Ë0õŒ×_D?ÄмoG')?©uÕÌ^±?ã3í–3ì?´J¸Sò:K?Î_7ìk*?«±ÿ²ßut?ÙSBeb>Ù?®×8ÁÆ?Ï!‹[^H?´J‹÷P"\?×øp?²Rq٘4FGL J0746.5-4113¿ã}É6Í
À 6‰Å!ÞÀ:«°ÿç¬À<IP«éþ@8ñÁ"õx@›²ãízÂ?ÊÄ3êé?µ•þk?ì«Ð¾Hûq@^ðTf^¯?ïþÖ~z¿ì@9
ãˆÑ¿ØOr"¿ßó«z=¿ç›#§¤õ¿âà¥Ç¥EŸUNASNone?àFz_óÞ$?ÁøŸŸ1?u½ßƒ±Ý?oïȐ·|ª?ßÂ	|F?Áêf;ŠÔ3?Û¼õÇ43?Ă@Zñýþ?p2ÿjm2?~ÏÑÂ1!?âRc'?Äm,V1lO?ç9Ñ|W$?©ŠJÂv–Š?•ZÔjVr¶?~b8`<S?Ð6¯À¬Pª?§ÈÖõë-n?éãmæ¯Ý?ž{+@üÿa?†:‡¥l!$?p¸ŽXÇ¿>?ʀÉÎ~w?ž7<
z(¬4FGL J0747.2-0736?ïÿí'ò/ª@!…–À:Õ¹Nè›À<MÓÔ(
á@ Œ-·c?ÿÚÇ犾5?ÏÌçå,0?ªå Å®‡?à(È
Æ, @Rn6êM¿Ùù–#ÃS§?×ƺCÞ&;¿á'àb*íi¿ÙEÉ7ìÖX¿çÂb¿¤?h50ìåy UNASNone3FGL J0747.4-0734?é§îQ€°T?¸÷ç£r€?cœL=m,?^]5hV/?ÉàHÌHø?¸µG¼ñî?åÛDǟ$?ǼðáÅ÷?lÐô¾+?|ÕàF»Ì?ÔԇÂ:q?Ǐ›
ä¸ê?éag^ ?¥£|ð¦ž4?ŒÄbkG}?tTÿÅËdã?È5DS®¸?¤—ÚÞu°ú?íb&©2~?'"
î'?€*ù9'#û?pzAÒ"?µ£"G'?'•£lȀ4FGL J0749.8-4420?å±/™ô;À"3󾩛À;9
£3vÀ<µ"6Æf@©ûv®] @RB<»r1?Ò娛•\?äÅýƒxñ@`ÔV.?òasÝó:Ë¿à†øaûó?UAª33¢ß¿»»Ñ«Xß¿è9']e5å¿ëUÛN¿ïÿýawUNASNone?܆þ«	qþ?ÃóˆÑéì@?Æ)g2ä½×?½6ê+Þ®«?ØdM»"/?ÛÕãÓº?ʯ6	b.—?È''›SP?ɕV«Ð‰Ï?ÉhVCIˆ?âîÜÒ³Qæ?Í73žâç·?â7ÚgnY?¯˜î_ø7?ƹx£3)?§ò'Å;¼;?ЀÓù¢	¹?§Äï–#Ð?ЊȾ*ð°?¨'çɹ?ÝãÊÉ4hå?´Pƒžžé?ёlx ¦j?±nNI{ 4FGL J0750.0+7140?âff˜T9@>>A€ÓÏöÀ;'u¸êÀ<^£ƒ'gM@ia ƒî@™æáK	?ÂZ	‹Å¿Á0'B]¼?ð֑§\л@QPiÏÒ¿æ{¼n°·Ã¿çýՃT´¿éØ·¡Â]¿ä´>Kë¿ïüž…¿ïï,"¹ºUNASNone?ïËěÍñC?|øÝ(.Eª?q!öÞæ¾*?uœÞg¬X?a÷vtAAÅ?kß¡™Bœ?îÁ¡pœ°±?£_­¨kó?wVÆÚ?Ž~»Er´?¡^s'²?œûî¸K¸?íðÓ{žK?',زSƒŸ?ˆÁOž\‹?zsšo:¹?ªÂt‰Î")?ŒƒQqD/?íÊÉôV'?š·6!"ZK?˜iˆeü?ctªOÁÜ?§*œ¯j ?•·ƒâz{4FGL J0750.5-7519?¸ti"ô7XÀ6ŽØ
±À;!n
#ÔñÀ<wñ8¼ßð@–'âòþæ@«Âßä?ÓʤzHF?ÛÞ¨éϒ@}€Ú…ó@Œ T‰D7¿ïÿR@>´q?ïû¾½?'?ì"}Š¿èîê.¤¿á‰ ]9–¿ïüö@
·#UNASNone?ï2g3Ç;Ü?¡B¯¹?í?oß3øËØ?h€!	³Ñ?•·3ÿ	?¡Æ堎õ?îÌ\'%Ë
?¢·‰$3?qÿý§›n¦?'õáòc? ú=دáƒ?Ÿô'$
¼?ì*ñÓÀ? s‹þ¡2?¡O@¨[?Ž°µþIó~?¶gdÑÔ?™²üðyêÁ?í ÂNë>?¡e4¢
?‰§/Æ`à=?ˆëZ*¥?³ÅÛ*?ŸáŠÃW»`4FGL J0752.0-2931?禘ÙçM¾¿ômY4N¼&À:¼&Œ[ÃÀ;èH÷À–^@]6fïM@]<9Aj?͐½'h?æêúêíID@^Íñ?ø~…—<¿Øy|ӆ¿µjF€þÿ5¿àùI—ù†i¿ë÷2ú(P¿ð?ðUNASNone?±Cì?©z²üA­?ɖ÷m¹#?ÇG.ésy'?çw·üº?ÇÔnXãá?°g¿²­C|?·€:ý¨˜ì?Ҙ7£Øåö?Ì⦻?ä¦ì7½ä–?ÌNZËë\?Á&¡lT? 3'ÿm©?àÓ´þü‡?²ô;z]Ú?ÕŌ2EüÇ?¯6£dØ?¶Ý€_̲î?žøVåçA?àA²E§AÞ?ºg‡Ïp?ÙÅ;\¾O‰?·ßµ¶ejØ4FGL J0753.1-2624c¿Ï€¸L7;+?á!l—¥À:ŸËz½5€À;÷ÏdVÁ®@ùáxÖU@1ìVuX?؀ÌÄjÁ?îܘQšýG@4' ÷@f"ÄB¿ïÿñò÷?ïÿ@Aä{ë¿â5¯^ý¼Y¿íLE¾P2G¿ïÿýaw¿‹4J_t¯ªUNASNone$?Ãܹ§7¤?¿Zön跘?¿‡wúÉw?¼kò<º?çâ–ðË?Æ\ñûDAÂ?ÅjÃ}íÖZ?Ǽ	Õq"?ÏÁˆY66×?ËV×®Ê?â´í
6ü´?ÐkČ_*5?Ø÷ws§`?­na•œ?Í·&	.?¬é_Òë+?Øz-E›b?®çI^¥?Ê­à'¼?«¥š á1»?Üs&#ßAU?¹ºèñÅ?։ë×vÍ?µª¬ç4FGL J0754.9-3953¿ë8'Kج»À?Ë~3ÓÀ:¢rúÉÀ<ÄxCÞ|"@Ž}á,U@?Qi›?ÌEú
G¬'?ïþ¡€Ã´Ë@öÇê弈@WzK˅z¿ïÿú@ùDz?ïþ¯¾3G?æiªK¿Û©q="ðÀ¿ð?íáŸËŒÜUNASNone?¿LÃr6Fø?À	ÙY‰½ª?æÙJ©^¹?ËAÁ³Óó?Äôs¡l½Ÿ?ÂÖò°ðº?¢ç˜¯&³ð?±•J²ž?æ9n—Ùµ?Í8kY¾´?Ñ0/ºg¾?ËM¡žðHy?À¡YR1?¤yôé%©?æ"d1÷??±pÚ­¦¦R?ÆÕåñ÷Û?ª'ÁÈÏ¿?«3ôé¦?¢•&Õ!Q?ìl?t|°?±˜ª®$?®	ÊÏ3U?¤×Sº}¦"4FGL J0755.6+1855?Ð%4õú\@6_ºº{'qÀ;]K´3xÓÀ<¡ÊVÐÇ-@´¦M@"Åyò4e?ОÖd¦à?yT¿"~ÕÕ?°¥ô›ÈÈÜ@~ù ?ïíL~Þ­J¿Þÿ<÷S½¿é­Wâ1»¿»uøÀ·¼¿äd¶Ê,¿ðUNASNone?ïÔ_æ?p´
»Äá?:d—æ›Vœ?6P)€q¤?tJŽ"¼
?oùkµñži?œ¼?"+¹è=>§?=G²ŠÉ?MÞA-u¶?‡, ƒiÝ?ƒtY•½¿?î	±à Z?'Ã'ÈÑ}ÿ?u§¯ÑñBa?e—ÓçÇÒ?¬º~ç·Ò?É9ÞBŸ?ïCÛ¾öA§?}äÌ?[€?v"LÂ?MÔr_¥†?•Ì")φ_?~=ãÄIŸ#4FGL J0755.9-0515?àêÏ´³¦`@''´·,RÀ:‹kÙlîÀ<³'àÚ@O—íÇï@ðù'7}E?¿µ2&mÒì?¨VL_KŒh?ãmjñ¢?ôäŠ$[ª¿Ïl?XÛci¿ê-Ôï°ýc¿ët·AË&"¿äü¦¯+Ò¿ïôèà(Ê$¿à†HNMjíUNASNone?îý«Fl'?¥Ñ½û­ý\?™'>Ue0y?¥)`2?öÃ?{/14ý?}F.ˆ]{?èܒ½n¡¤?È©»PÁœÐ?±~~ޜ?ºVK©¾Çv?ÃÿõËCŠ%?Âéyê¥(?ê`—Ô;?¤Èbth?ý?¨—JóÖ?•Ã‡EÆÀ·?ÀWÑ?êH? 5€Ü(?êX&+?ªÜ"óB,¦?¸€#}¶³ü?¦C¶_¨Êß?´¹ÈóZ?œ.Ãg±(ª4FGL J0757.9+7304¿ì_)ßU@>¯½¯ljÀ;Ï1_œÉÀ='òH‡XN@ šj$"?ûÁý¶y¤1?Ôp†yÇ?Îø" 5ª‡?÷*ÑJ
M@°sAI?혬3Ð%¿êVg€AÙ¿¿Ñ
7öçRŠ¿àëL4"†¿Ñ`Îvðø%¿ïÿî,˜å?UNASNone?îX_ÀèìV?´ÝÍGø]n?më"g~¨×?p±!	 D?¨›QÊùP?´¢°›íÃ?îÄ=ìBN? mⷁ?l
ÚåÑΐ?z?Ċµ?¡ûs~4?(ïÇÉ%?í2Ñ?›»+`jь?ˆÔ$±4yö?€E"Ú×-Á?´ê"Qp?˜ˆ~ÒÒ7?QmÉ?‹GèK¼(È?_Ëi»™÷?Vø.)Ò9?¥«€o›F¡?ŠÿÛÐÙÄ4FGL J0757.9-1514¿ÂrQ²‹i;@ë¹]"?•À:?eóSIÀ;Üèi
…•@T'ÊtX@ÎíEé]?ÌɞÄüžÍ?ÚX™Ÿ"ðp@
2Väé#E@w5Êè2?ïû™3BL¬¿áŸ
='¿é¾kÀÃT(¿îÔÚbaŸ¿ïrô^Œ'k¿ÐÚáŸÌUNASNone?ëŠþ9›`¶?¼oÒX…»Â?ª¬ڊ?­·>©n?¶Ÿ	Ñ΍?µŽúuôu?Îv༭Qa?ÆÃyË€?Ð8@L¸UÏ?ÅÍ'@?àF'ªx€À?Çèy'h£?ã(½}/X?±qÆõOŒŠ?¿N}Ì,}? òãøØ|Œ?Ñìq?'–/?­+P½<B6?Ì	àي?§»ðD™•—?ÜcAÿ€Š=?¿"'K+S??՘2óý?¿á`ù›on4FGL J0758.8-1450?·£Ôz˜@sÞ¤e¥vÀ9éɼw4À<O‹À@Y{SJ?ý–ç½éÚû?ÉÁžÛÍƝ?â¶ÝÂhoÖ@Ÿ=áâއ@rÅë‡"?ßcøb|ÌÚ?ïàuöý!ÿ¿Æ:'v_'Ç¿äÕub'¬¿î"0Akˆ¿ïÿŝƒ‰UNASNone3FGL J0758.6-1451?" =쌚3?ƒÑý^ôþ?í~›ï^?µIìË
€~?´ðbõ¡Í?³¼mZ{ÓÀ?£úc*–Û?®–?ˆgK;?è™FBÌÈÊ?Æ ¬õlpŸ?Ȝ`\7#?Ãބ# Â?°µ"Á½ºØ?–Aä5ZAU?écY]âX?¨Rt'ç?ÃW¨9©™6?£œÍ ã^ê?¾ú¶ëÝÛ?¡lDeZ'§?äØ´³ä.ò?µÝÙG=Ò?Í #TùUO?°­ÈD&Ç4FGL J0800.1-5531?áúÜÔúHÀ*@!ÀD(NÀ:Ìá*?À<ªGfÆÞ@ï°oÉçj@ÁÅg}¾?ÉÄ
'?–%"›ìÁ?ÑXŽß#@ÓÝ¿¹>?ï"¸Ç\J"¿â@!X?\¿ê
…/J¿æBM'iҿדrãø7Š¿ïÿ'ö֌UNASNone?¹
Û? %>0'?vCÓ6^H?pÏ°Êx?£\ú'"ø?žx;M¸­?î4mbÿƒ??°ðÏÉùq?^Õhyëx?nivÿŠ6?«Â~Œ?IJ?°¸—§ã®C?ëðêQw<?£q'غV?Ž31€#ñ²?z²E¢¬ô÷?¼²GDA ö?¡Ú
%·á?í)#4+cï?•l¯Ò§í«?lç•D#†M?_æ=9"˜?µÏ©´ƒÄW?•DKAì4FGL J0800.5+3715?Ù{Ázf×@='à°«À;¶–ʞÀ=jïVd£@Q±; è@¤+eßWê?֖©ÁÍ?ïþh@0FÅ@
ˆ¹w…s@dCðš²H¿éŸù8¿å";‹ÇI¿ÈE/‡­¿çTÁ£Mø¿ìrô´rbô¿ïÿ»×²UNASNone?âÛ\4Îðx?ʲ0<č?Ô¸AýX?ɕ*?	?¸¾=Q"bâ?´i2 Á¬Ý?ÚùÎo?͘E¶Ów?Û´-Ž&s'?ÐTĢ†?Â¥Ã|?µÈxXÅûM?åÙl/Õ°?¯ó¯åJ=?Ĝc4ƒ?¨4®¶ÓŒ'?ÇP7K.tÁ?¤404lGÙ?Öâaì¤W?ºŒ7°ø?áû˜X&?½m8VïB?´ƒ‰â ?¬'ðœrӁ4FGL J0800.7-1059¿ªþØÙ7£·@#ú£iüóÜÀ:Qû]ÙÏëÀ<9¬üLí@×Õë™"@ŸNìő?Æ	[ˆçÅ¢?ÅAòé—ï?ý'-K6?ü/š.êÏ¿ï²LîÆÙ?ïÇìÞe%Ÿ¿åÏ/!}¿åNžsž¿ïö§ý	«z¿ï+þ¶~ØUNASNone?áø€¬¨ß?Æ©£ýÚg¸?¢‹£à+? X;IVù?Ù½Š+ãK?ÆÃãce¥µ?è¶ÝN§¾?ÇgÉ|Do?µX
/•ð?½·'}%œì?ÃUsD–
?¿©·4íØ?ç»Å'Ýí¨?§î®?CŽ?¬oWþ‡gÒ?"'ㄺ;<?Éõ`æoj?¤˜®bØ?çÓµT‹Ä?ªw$U¨«?Á•ÓQ\uy?§Vˆ)á2?¾<+²¢¶ð?›œÔõÛl…4FGL J0800.9+0733?풼È?@Õ@2ÜJ@•òEÀ;~™Pž~À<éö\é@ Ž¨‹úʌ?ö½õ<ó¦?ÖHì'õ"@?げ©@ûA3¦ö?ö~ÌôºÒy?åè阵n¿ïÏYÚféC?ïÿÊ»z"ò¿•Ã0}¢¿ãÍé,~ä¿ïïá9k[™UNASNone?A	d?¤i딲¾ø?:§¾*6Ñ?Eoz]?ŒJÉ·ý? §x(|9^?è©o¬-Ý?ÈVÿƒ`KÖ?³NèY¤-?½Œ7çÔÕx?ô"?¢vt?Â;CK™?ê'à´zu?¨ÎC椢?¨®¡Á"wR?—
`ÅØ$?Ák¸É8X?¥Ü¼¦¯?çÕü™ƒ¶?´cºDÁ™…?«U2˜ô?¤! h€¤?Ìû[‡³´?´|‰È§4FGL J0801.3-0617?ê–zrY[2@(èä¸{ÜðÀ:ŠS±WüÀ<s'È@ùº=S³@ ƒn—?ĝwI¸…Ã?œAí¤ø?Ö–­V?ü»%_5?ê?'—•¿±¥Ku쎿í3Ðçå¿Ë—¡ò®‰¿î#f!/a¿ïü]°	sUNASNone3FGL J0805.0-0622?êx`|ûÚÃ?¼£ˆmæœ?šYtNp0ø?•Qr7Ô?ÂÓO'BŽÙ?»Xo–Ž2?ì¨ò«U<T?½H#됋?"qð…?˜è‡L, ¯?¸*GSÁ?»-®ÎÅ{?éäE	Lœ?¨.Ê׳?£™w'ä`'?iZ–&0?ÉA!µ‡?¤ñ¸^˜?ë©T±FL??¢½…êU[£?ª@³Ä"Àâ?™±´¸—?µ•"ƒ½?š·aÄXU"4FGL J0802.1-5612?ï+ñ-‡Ö+À*kQœIwÀ9ÑÈDŽŽpÀ<Wí|o½'@
¤þ&¶ù?ÿ¡Å'U°6?À]¨½#ž?èMàÞ|¢"@#sÈ:–ÔÃ?üüo'ôn¿éÉ9d¥œ?Ðû‡n…D¿Õ´`$-ó¿ê$ŸANSö¿ïÿýç!é?èAôl#UNASNone3FGL J0802.3-5610?´Á)·å?·+åì×	†?ë	Lç/e?ÂrÉRç?³š'¿œÌñ?µí7$"…Ó?¡íŠ‹%5?±=
HQF?íb Œ<®?¶Œo,S÷ù?§èuW±î?©pó?«Å+†/?—gFÅŠ?ê8bÉvž?§#žÔÅÔ,?À-+=ø™Ç?¢lX9"?•yªè¾ã?…#œ…»?쇂£"ð¬?¦፶¿¤?¶eŠyJì?¢×ÁxJ"4FGL J0803.2-2522?±Í"Ç…Œ³@ùݧ¤À:ãhšô­À<0ãs\@…_ KúÕ@ª¬Ùè>B?Æ2šÜ垫¿' ƒ~áB·?Ð0¥Nفç@b"¼î]k?îR¼›&b¿åîs°Ñă¿êM=Ëg¿Û!L€â¯¿Ö—†"iÓ¿à"ÈŸ@¢‡UNASNone?Ú³Mú9?ÈÉZcjÞ?}v£k‰;Ê?q¾ƒÛb
æ?âÁ9hðl?ÖÐ}™³2?ážTÙÆ5?Ê3$ä4nA?{C²LVF?‰ç
NÁC?ÜVG"bd}?ÉÙ)4gB?çk—XéÀî?¨Ø›–×?'Ýì¼qŠ?w5¿=X‡Å?Ð
ò'em-?§¯F¤Ð?ëüˆÑ9{?Î‹ŽÞ?tO"ß䨴?f*&hóÇ?Á'=»ôÎ?`D3K']4FGL J0805.3-7425¿×í¢ðÁõÀ5QŸ<pɗÀ;8rǝ¸ãÀ<‡TÂÏóÉ@x4`YÜë?ÿO²ZZ¿i?ӊÙÂÿn‹?Ôb'ÁÙ'?üµ]åŽd²@T"Uð¢¿ïû¨b4R˜?ï$‡nÊ?­âcAën¿äO
?¸¿ãÏJ ¸æ¿ïú;e0ÜAUNASNone?ïGY0³Ôì?ŒX)m>±?hxŸy?aBfùâ?"ªæQ¶?ŠÐûã(Kž?îæ܄«ó?›ÏºÕwn5?f÷"¹±b"?{RµéÜûT? /øü*´?™'¨©/5?ì™t±Ø;‰?œ«œ;/F?šº×Q(&f?ˆŠlBÿõà?´…¤œô?–ÍŸ+² ?쵓?—¬0iÑ_?'ª³sÕ?sŸœÚ`2÷?·þ»q?–ïZºk¥4FGL J0806.8+5659¿ìÇ(B´'@@O+ý´Ì%À;¬sè/(âÀ<ôe;Ãûm@ Ó{d¥F ?û¯W™?Ön5Ó £ä?ÅöRT"Ö?ñWE+ƒ;‰@ï¾Î²U¿ïÿêf:Ç|?ïÿx†#›¿çöˆ‡ù^%¿»ñöýÍË¥¿ïÿ‰î*ëf?ïüÓZ…‡"UNASNone?ïãÿ3ç[?g"€©¹?OtÇ»çB¬?Pk2ÓѨ?e ÎÝÓÔ?ci3{ušº?ïAÀûăw?•^zKÙC"?^˜Õö@ ?p2W†î?•ÞS(ˆF?'ÙÙÅE?í{Ÿß¸?™ööÌG;?yD<ºD?`OõÄ!±?³ä´úyjï?–­ù¼'×s?îĝ±¦Â?.âšÒËË?s¤Žø%ú‰?pûʲô?¡JDEàԘ?Üw¯Å4FGL J0807.2+3312?ïY;R@=q
{é…jÀ;{ë^ˆK"À<Òâ'0ïŒ@{;B `ô@¡E= ó?Òå–È.›?Ò¢
a,ë›?þ$Ü=ƒN?ù<p>–©?ïþ âx°–?ïí5€†£¿Ë¤è'4ù¿æaµ&½Ú¿à_•'Í~¿ïû…LXžUNASNone?ïEóۃHL? b3uú·?t]ÌB+C?«ôéPG?'* œ†k¤?›ŸP«Cß?í«­0*ô?°G^ðͬÁ?™¬³à7?¢ÈÓë/Eþ?±wŸÔ'°P?¥•Ný,ÔÒ?ë<òC@·9?£«SŒ|v¼?§öl#r?"sšpë?º7ØèÅ|?œö½EcÌj?êxQ—;]Ý?ªìžÀÁ›?²±¬Ñ.¹(?¥`\ò
‹?¹‹ÆtöWð?¡@=^Hù4FGL J0808.3-5121¿äQÿ^ùÅÀ#ñÆónøÀ:p1ÆK©LÀ;ܽ:ˆ'
@h`©
*
@
	Ö¶[?Çî•ßе?¹–UGì?ó~5Å´ª—@G+ÇYx¿ïZ쐰½?ïݍyЦv¿å©mƒÐ¿è×_Y¬Å¿áWÊÂ0'˜¿á2€óUNASNone?ÞÙÚ€…T?Ü\Üú…F?†—yct¸ª?€`²ç`Tì?à8µ1ês?ÝÏðIb†?éÇe€É¼?ÇÒã
LQ?€|I(p°Q?‹a±"Éa°?ʝ×uÎ?ǛV­x!%?åÍbè"ud?°F‰²ÝP?¡ø{L!)'?†r¾À?Ò&*Årð?®†‡ÅÄû?æ±X¶ý?¦`Ô©m×?›îÚ4âà£?‹Næ߁?ÐÞbUC×Ö?¦J:XP4FGL J0809.8+0507¿ê‹µÞHË @3Áõ8%á;À:ˆ$?ziSÀ<@w¯<™@iIºß™@…N{ŽØ?х¨á`,»?ëtm$ƈæ@× eeµ@	ÒG6u\ù?ïþš¥2T¿ãœ \–ÙÌ¿ìÞî7€ ¿ë7ë(Øf^¿ïúžâXÐ&¿äC<àÛødUNASNone?í¯Ùx[—|?¸Ÿ»ÕEÃ?±DÚþÞ	?¸]8%£MM?sœäS±9?|BMŽò°?Õ™§Á?ϐÃpÁI‹?áe§…¶Âw?ÑMUvåZø?À>.™¢Óÿ?µd_ŒµºÐ?äUI™µ>?±¤Õ¶èS–?ÇòŸ"‡9í?«7¯ßì?ƹ#·ñ?ª©&œ	Û?ÐÙ®Ž>ì®?µ>¦s?â¯DÞ^ej?»ú<DÛ¶_?Ϗjü?«ÖVgíÑ¡4FGL J0810.0-0505?êuMÆ@-Ùh">À;EìSzÑWÀ<˜(=5ët@h
0ëp?úÉoŠÑ€?édÝÀ$5?á¢ÛA"¯¨?ù·$#Ë·#@N²OÈë¿ïüœ¾g.b?ïåèâ­â¿ãÊh8Î}§¿ØߕÜö–¿è$½"Zm4¿ïý'!« €UNASNone?í]nÁ <†?ÆW€bΞw?~\âOÁ?{ÑÕ}©½?³*´(ÖÔ?Æyÿ`Îs?íÐÑW|"ž?²:~Ô¨ë?…ßüâí:œ?•êp7³ C?­zëO{go?®ÿ{5²Kø?ì:@ÿ
? é‡Kš_X?™4F¿[.Æ?†©õÖÝ«K?·àé`1ò?jk4&{—?í]ÇVnSÁ?¢LVdºð?{ÆEMƒP‰?‡C'Wñ¼?³U`÷µ,ñ?¡Åim54FGL J0811.0-5636?çÝù<cÖÀ(´Jb#á‡À:&Š®DÀ<öÉ™"@i¥ˆ€@«"}¨¢K?Õr4ÐÂ$Ó?Â'}mi?ôò†š¹T?þ{ZÚ6x?ïû":ŒÃÈ¿çÑ;&F»¦¿çM<>ɚ¿ÖôF£ÓYY¿ïÿJ˜ª†Q¿éyéÐé'ÿUNASNone?î`ÏïK'?¢Ü_d}¿?pA!_ÔVû?a#+7¹5?§õîÕ¢?¡ÍË%ìËÌ?èõû~©Ù?ÈðŔR1?{MHѪ?ˆÂ±ÓøŒ ?ËK)ÊîU(?È¢'êõý×?ëÂ)0A?¢4"^!?•–ÃórÈ?"çõEE¯¨?¼‰''¡F?Ÿ´xœ0d—?ë?Bԛ3Ø?¢¢ƒ8E#7?Ž¸¿=¾`ø?€Èàj	Ÿ?Áh¹·JŽ?¢3؆(–4FGL J0813.1-5049¿ãù	Ž¤À"">À:W^!ôFŽÀ;¿jК¸@}ã ÷€@ü*EMçê?ɂâˆuÚÎ?ÃùGÿóë ?ùlsßË­@·Uê™?ï_‰ÓRù¿çt¸Œ£è¿æŠP†*Q¿ì	ÜW"KT¿Õ©ºy
2¿ïý3!jˆàUNASNone?ÙIþ¼YÅg?Ý;Y}%?žgü°\—?š9ÕúæUq?âgȉíšg?¼‰Û5˜?ÙFf./¦?ɺLÔî:_?&×…×m?™]Ä ‰.?âè^ðÚÐÐ?ɔªŠØÛ|?ã2à•Ø¤û?®0¼Ùq?§æßâ?œú›(Õ?֝bñJý—?¬¯Õ_'?ßÈîã÷Í?®
‡›
?™B½ª²5?Œú|-V\?Þ¢åJ½‡Õ?®/ꃶ›4FGL J0815.5+6554?æÂ0wÓ@@'Ò^ÝÀ;Ýh1AÁkÀ=ûG3›8@!´u»îÙ?úÌ 4Ríä?Ñw~ý.?»À'׳…©?èÝAÄÆn@†újê°?ìDS­úпíđʘ?'¿È"ãw3=¿à·íu?¿ÄÓàR:µ¿Ü+Uc‰½.UNASNone?ï\…àȏ?—<w6>î?N«&«G?GÔ©aÏq?œß_m¸¢?–óî¥îT??聾Ê\Ú?›¨lsû«?^ñ‰<«Qå?rô\áð?›¼6²é¯­?™q•ê
Ž<?ípàI'?™ð²9Yy?p9_ž4¬Ó?iÿ4K#­	?³|;Ð-?™&3þ;?îà2ßZ™?ŽÇö½ytå?LÐhۙÎ?H	¼xB€ù?¡‰fè
˜?ŽÖ&:ÒÈ4FGL J0817.7-5258c¿ÑY+'LmÀ#:1…ýÀ:[6ÖUâ‹À;×ê¾O@8°.†{/@CºkáÐ?Úß©HcF ?ç/Xb—¤Í@Õ¸~a.ï@=Õø¬¤¿Õ#lì'dò¿Îv~6'·x¿ë–îÄnYz¿ê{åßBp=¿ïùV}»¿ãs_ÍSÛUNASNone!?çöÒ@††?ÃïК"Š§?Àª»(·ø?¼h¬ïù,?¾õl…zÝ?¹?©ÊèŽ?Ô:c¢ŸŸ+?Ë0üWg7F?Ë
ëû<ç?Ç\p×v??Þ>¦_×Ba?ÎñÔA?ã¾Ù<Wx+?±o4cri?ÂÈ¡UD?©ÔS':a?Î;ù¹‰ÛA?ªXá‰k©?Ö¸¦Îšn?³	q"ái?ÑؖM@?¹…6–š{?×oaHä%‰?º/dµ%°4FGL J0821.5-1436¿Þ.µybÜ2@(×bùÊ[ÙÀ;\>GckàÀ<ï/a›M@C×Æ%ß@*,©¬6T?ÔõD䋅?íâ_ !¸@Jùe²€?û@»×‡ÿ?ïà/€ KÐ?Ú,¢'¼†¿Ý¯»/¿ïáB‡N=?êŒäIÁ2¿ïôþ¯çÝUNASNone?æ'L‡´®?ÆØ57qa´?ÂaSëλO?Á ®…7â?ÃUyõ`Ýø?½««Kè?àñµ0?ѳ·`ñßZ?ËÓWÇ¢'?ÍOï5´'?Ñîq…Îy?˝ÙkðÀü?àL‰Ó²-?µ)."3—?ӂôF*?¶—¹§3)?ÇÉ°Ëã=?¤žÏß |÷?å²Wï"X?ÃщšJB?Ãx¨À—?ÃûÆB?Å¿N'ß‹?·ðêïáï4FGL J0822.8-4207¿ámR_.ŸâÀ±ÕQ֌À:4®'xbèÀ;twlH(@!fø1ªr@ÆcÉÓô?Ç^«œ{vC¿ VQ›S-$?֜TŸi'@@X·ˆB[¿îø–^ü³?îqBÝöð¿Ýû
'ç¿¿çô¯¼пЈÊÿÃE¿Ø«úú݁PUNASNone3FGL J0823.3-4205c?ßӝN*‡?Ƶ´¹:ïÁ?U€Ûx/²Z?T¿H"Òa?àpë.¤œ?Æ·HÕhD?ߺÄg©íŒ?Ï·lÆQ)?^;|wf ô?zAá²d°{?à€
ïUé?ϋŸdËzÚ?ã5Å"IÞb?²¼¼³ƒ^/?›•a©›ƒ?‹©kÒÂZ?×Ûª!©"?±Ü¹H0®?æÝ£8:"?¯÷ÏñJ\å?fE³¿H5?a½8r|>?Ò.)ÈJ?°
Û9¾Hñ4FGL J0824.1-6004?~2áì©À)wùÖñýÀ;W†Ç.þÀ<ªZÉz1õ@!ÄÀ:Çý@üÑ\~†?Ü
ËD·j?ïÿ±eh@.Ý}ôøe@Jöô=ª¿á¼œ2Ñ
¤?åRqâpx
?·sëÇkd?îÙ²X­@@¿èù"»¼Q¿æ‡Œ+ÕqUNASNone?êN¢øã.?Ãs'?½«îž¤¸h?ÃscÛ´(¤?¯½ó4…<T?«a»r
†å?æ¶Ê}Q›Ú?Ó÷MT|?ÆëÊ櫃È?ÐÎLP¸¹?¼rH¡?Âx
Ø,e\?ël)ožú?£Ð	³AaÂ?¨q^;P†Y?–ËMoO?»›ï–ÚÅ?žÁM—,Ì?â΋Ґž÷?Ì÷f¹jº?Ôí¡Ö¬?Î`hÔ÷Ã?¹Gí0ó­œ?µ©5R ç®4FGL J0825.6-5216c¿Èä9RNÀ oŽ\NµpÀ9¿MÈ	ïmÀ;Š
öÔT@/A:2@'âƒw?Êy@ˆ±>ý?Ó¶h\_ÒN@Ç>Ê€Â?ö#õ¶6ˆ?à*ڟg¿ß]e¡DˆÆ¿ê¾'¢O¥¿ï'Iž¯ƒ?«ØSœ<ê ¿ï•Û¿-ý¿UNASNone$?Þà†x–¬?É·Ø>³?®"ëÏM,?°ñ<ô.Ö?Þ .Ü
®?ɜ
^£ÿk?ڀ€çv¢?Χ2K·?¨C!G˜W?°oAè;r?á?[Z]Ë)?Τ;ƒñ?Ùt®øæ?¯¸s'-í¤?ÁæjÀï6}?¨Ú\–£$?ݘŽ~©?¯¬³b+,è?áS>ùŠt?¼néát¿R?®í,JžT?§"8ÒÃÓ?Ù{܃º7O?¼Ë¦pä^ê4FGL J0826.0-0157?ï§'§
öc@3öˆœTÀ:­`#VF^À<u°ç"øp@ÜÞ'h#Ö@DÙMä?Åßïÿ¬Èö?³íDfŒQ?í./ˆƒÇ @ª6+‡m?ïýI1¢9¿ç>¨Fۆ¤¿áüHKá¿æøÒpXƒ¿ãÆôµ¿ïÿÓ?,» UNASNone3FGL J0825.4-0213?ï¡w"Ìy?€ÚªÉÉ?JÁ¬€×Š?DzW—P~˜?…öìè÷?J\ŸIœº?ïu()¤Ðé?Š]‹Ž~?QåÀ¡ûç2?a!ÖäÃ?<žÁF$b?ˆÐ²·Y:î?îV ËË?Ž?›ìÊÌp?xŒhœ!®?héËÀ	ì‹?§Œf;ÿ''?‹•ƒ!H·"?ï('`ñý‹?yù_¦è«Å?rèSõT?\}i©ï¾?–lyÌùQ7?wóÉu‰Ýù4FGL J0826.1-5053¿îÔ6}jÀŠòQÁ"´À9ÝË£!hÀ;©Ââæ@ž3×Ú@I6'sg?Ä!Z˜§×?АA–£E@
Ä.bT@kK
¶!¿äïv_Ø­¬¿æðÉ+WœŸ¿Þïeþâs¨¿âŒèæÞÆÊ¿ïÿž ßt¿è««Ÿ«yUNASNone3FGL J0826.3-5056?Òâ&ýÜÈ?ÁqèaOÌ?¶a…ÅX?°oN'Ü~?ãÂÚݘò?´ïÊÓ ?ÓÇiIþS?ÆÛ8‰kè?£ýVÊ_£ø?©(…,I‡?äܟ޵—?Ç>¦'Üe)?גmU?0?°	~µ`q¯?Ç÷ðL¾%G?¦"K®ˆÿ/?ÜqølK®,?¬·\y…©¿?ÚX3°f\V?±îHɄÿö?¯Q6ùaî?—í
'&?àÞÎ4];¶?³kÝt74FGL J0827.0-4111c¿Ð0îáZ߆¿úköÉ™"À:"'‡V ÷À;‰Õ¤â¢ø@!«t0Ô^<@dïmâ?Î`R»Ž¶è¿ŠÄ©Šô¯?°:³ží/]@+áìõ?ã@JÞJ£'¿ÛçÚDY¡1¿é°Úþ¾·¿áírÊ!÷¢¿ÂN9žÝ%`¿ß¨bÑÜVUNASNone ?Â=|nY' ?»å8³p_š?a®ÁŽî"?dSý0öîA?ë^ò"Ú­ ?¼Á®tøó?Éä¨h}ùj?Ä:LkKY1?s½c¯ÍËð?ŠbUQèÝ?é_[€æ?Ęßò£8?×½Íé
2?¯ÆB®¦œ¯?¤Ñtktª[?Ž‡¬ÙЮ?âÔÄÜN?¯W#ëÀÒ@?ڟ
×±õ¶?´CÛ5dÌ?n9vi›^?j¬"
²,?â'A½j!?´cK˜¶34FGL J0827.6-0059?å~—eóS@4Å2¤—ú]À;lWÛÀ<™ã½ª@ 
ããê¡?üe2.?ÓÓMÅZ½'?Éۥá|?õªŽI@Öې	"?ïýÐ_ÿD¿ß:Ç|*óÊ¿æAIvk—(?¯Kì_ÁW¿çIéXÎG¿èsHÎ÷ŸUNASNone?ï¥îQ!'‰?}$¤•˜?M&‡"Vv?L'"6üpe?"²ß-8+?{åïµY|å?ï–?ÆîhÝ?…­­Ç»Ç?GÜotº…1?X+`??ˆòGM +?"d¼O*!?¡1%?ÃÝèIN?}'vŽ¦äü?sƒI&àC²?ªb¤?Ž)чn͔?îê€õIv?…L"°³P ?eéê'Vû-?\£¨@?Ÿò¤"'â?"Ÿ¯V5y84FGL J0828.4-4444?Âù^6}PÊÀ ¸Ý+¿¡À:|ÀØ£À;Ï™¹z
@ ÔÊCX@é@&?Ïø‰ÿr¼`?ë:I½cMW@:ð
­@]"N+1¿è¦î·`-¿íù䒼/Ç? ¼«³¿Ý±cºº|¿í½tŸå
5¿ïÿþÞ÷UNASNone?kL3bÖ?—‹R?¨?'?Ø1ÏFÒÙ^?Ƚºäœ;?âþ½4ø9?ÈÁð9;\ž?©ƒL'[J¬?­ºv<;"?ѶS	½:¬?ËÈuW\?匡¸«­ÿ?ÊçÙçu'?¤ƒ[^?£²Ê8K?ßæÛŒd?´ÏŠ^ ¥?×RyÅí?²'ÌB"?­@c˜«?–»uJI??ÝÀbX(W?Àr»W]Ÿ?ޗ[d"ž?¾²°Ì*×*4FGL J0829.3+3729¿ã¥ö!vÿ@A`mqóbcÀ:Œ»NŸ À<xÉÓI@§6õŠ†+@0ïVd£?Çá£Þìßè?ѐíBäE@Mjßqêÿ@ì؜¹´—?ëG™ò"í¿å¥Ì­ÃJ¿é¥ß™±¿îå7&ݺ[¿ïµ6þ™Îs¿àЏ¥UNASNone?î£%_VV?ªVÇ¿Ë,?•™'.í}?"‡. ®œb?¤I"d?¤á'çüÒ?æã–À28Q?ÃûmßíCi?«•›!f¦?À)«¾žv?ÁÆd¸?²¸¥âŔ?é-Ç,÷?ª"±jÒñ—?±é5mš×b?™_Ï­¨S?ÂVî,Ñàu?£­€êf…?æ™qE)"ç?ªË­Îù?Ɩ¬ÂŸ>÷?¨³þUª'æ?¾Qtâ×?œY¼A}ü²4FGL J0832.2-4322c¿àáµó8À<œƒXåtÀ9˜4¦Ð¹ÁÀ:‡l¸K@ ½[8á@½·B÷ÌU?ÊV/wˆ¿g$b­@¸?¹í•W?@YBkàMÞ?ïü÷™Ã
¿èË÷º·!¿ê…ñxô¿å MÈ௿àùã»üšñ¿è!,À¨QBUNASNone3FGL J0832.8-4321$?³ÌãiÀ?°vdQû×õ?†…"Îgd?†gREXÍ?í3ÐPZ†b?±j–׏
p?ÌXbª¸?ÂüG"z?€_€â=pN?'±/ž|{?è¨iy¶'?ÁÀ‹è«õ?ÊsÎÛ$mT?¦NNÑ~h'?°ƒÂåü0ç?'<\‰ŽC?çR"ìw^?§­X|¶ï?¹«xªÛ?¤X¤ øº?o}'©äoX?aŒß½aJÈ?ì«ÃyV?¤C¶ü,04FGL J0833.3-4342c¿Ä¯áQ
¬À—)|Ñ÷À92\ça£‰À:T@ ¤		>@Móùa€N?âÝÄ6%Uû?Ôñ†U7	?ò&˜Ö%;#@í‹k®yÐ?íYÌúïõÇ¿éPCD"nÀ¿é$ó¿ÕÃk¿ß.^b6¿ëÏ*à~Zy¿æ‹¿m"¬UNASNone ?¦A…£â­?­‡"@?uõöëÚ?€\]ýõô?îqã¹Óý{?®†¥&±|?В¹Ä'^?Ã`C‰Ù?'S)²¼z?"~ž˜bï?çmVw4Læ?Âõ˜Éøj»?ÕQ2Ǎ#®?±-ÙÏé¥C?Á/—kÅ?¦ƒsÖS_t?á†Vӓ8?±»§Áwr7?½›H¸þ|õ?ª¹£:*ß7?\ž7"²ë?b6Ûvh?ì>GÍÖì?«@Rû'4FGL J0834.9-4612?ìÞYHÌÀ¯"9櫛À9G6v¾À:¯"½i'@ &K¿ÆÿÙ@q̾Šë?Ëjß\qp?¬)œÜo,3?å¡ä¶Î^?þö-pülx?í4T€ŠÔۿ뮛‰]â3¿êj •6^¿á?&¼,k™¿ëPݾ¿¿â†œ1#Ž{UNASNone?›9ŸÃ_<Ã? ƒSÔ'2Ì?tÀ«‹þ?—¨üh*?î¨bæâWé?¨¥ÊgT…V?ɘ«Aëg²?Â;-x?–ãz%ËH?£~<Ú;Æ?èé¾³÷¸?Áü6Õ†?Ãw4?£fœã-?µ×}ñâ?™qé:|
V?è"ƒ>U}?¥ÿ~ëGL?˜E6Ê-?‡W½.°®?‡Õ±wµV	?xS"À7ÓV?îށ)wtV?ŒÎë9h4FGL J0836.0-5458?ÊÌÂ×¼¦À!	(¿;ê'À:SEùßTÀ;æÂW(@A&œÍ@ˆ!¢7?˘iñŽM?Áøü–'O?ô½áâއ	@Ûr±Î?ä•qì¬f%¿äègÝßÄ¡¿ë¢_:øú¿ã
+Í
dm¿èÕøÅy¿æ¤O QC¿UNASNone?ÛZ¡Äþ?Â,ä?¨JŠíš/?¡Zä÷Ÿ#\?àÎKo$^?Â¥¼%>?á¼K hÍ®?Êg–FÍ9}?ƒÛF/!?±·áÀn?Û菍±ëš?ÊCWˆû2?äJ§Ö/¨'?¯u݈Я?§mx_â?ŽE o¤]G?Ô}Q"²¸?­
IAoÞ?êJàR¯õ?œ®ßà¥E?™³ÌPlŒc?}ß*pŒ?ÄLZô§®¢?›-œ[Œ˜À4FGL J0836.6-6036?ïÒÓ:éÐÀ'õûmÊÀ;ĘÚÀ=Q΁ز´@ÙÁ®‹™&@'$·omv?Ùè—ä7Íw?ïÿºà¼ô@zœ™(Z'?ó¶Yh|O?ï¬;ݦ¹¾¿ÑÏ£@âH_¿Æº–ê<Ê6¿Ù£C;"¿ëØMú^Ö¿ïøg_µ0UNASNone?æÞÖ«GY?ËóÛã6€C?¼LZŽ'R?»,dÐ‹Û?Æ^zç™s?ǬÑ$w;j?Á5¡kÏX?Åv@ê—~A?ÙØCǟn®?Ònñɕ?݌ë'Ú©¦?У>«Ø¥~?ã ùџu?±9ù	&S?ÆmþIªâ?©(^h\ÖÅ?ËÍϛ×J?¨ðåŽ`¬ï?±,]ìg?¢ÇÐ""á\?ësU"Ø?³€ð°Ig?²Ø*‹S¤Å?«ŽwI54FGL J0836.8-4638?ᓋOûôÀ»Ä?_'À9m.Y°À:°ËJì\@êv¹DÚ¥@<G䛬?É@tú¨Ó?²µÔ¶a{?硅‹Å›€@ÑQž?ïò÷ÙÀÑ¿í
°'z˜M¿åÆ ©T¿å³Æ)ñk¿æÁqN÷´Ø¿ïÿÊ»z"òUNASNone?ÐØ>z§Â!?Â<sÀÔ?ƒšŸ&Tã4?€^r³(ÎÆ?çEvFËc?Âg{rá¢?Õ8»'"ۏ?Ä'ððà?})wË1=?½¯Zó=?å)mãÆ{Õ?ÃÔÓ;ÝÕ?Ø'y3hþÓ?³†ÌŒ?«©žá€VÈ?"o#}§®ñ?â1©x3{)?²ˆO(1?ÈU"^[&\?«(oÀ8§?ƒwºÎà2Š?qÚØ-ª<?霼=-µŸ?«]šIs˜4FGL J0837.8-4048c¿ím@#ì'?ˀ.¤SAÀ9M1áú[À:µƒßóðþ@~;Å(@6¦Bˆ?Ç×Ñ7À‹¡?Æ$£ç"@߂±ö‡±?ë`s/¢"û?ïýAԋ³¿äè]_V¨¿çæ끘Æá¿ësP$¿ð?ïÄT=nöXUNASNone3FGL J0838.9-4056c(?á^ç5G&	?Л6>_î?€r{¢–?¡ &7‹#f?ÜZ
'ÝÖÛ?ÐoTQöS?²½×~w?şĜ?!ß?±2l€K??µ˜ÀK­Ü?éVÅÀ‡¶û?ÆÞ'&ÈW?ÑâÒ5ªV5?­=hÐzW?¼§1q¬è©?žß¥ƒ^4?ãy°¶õ7Ð?­ïÒrN?¢FÎ5î?'¾¬¿§an?¹¥ú/ÃÉ·?©Ùòcô=¥?ë¦à=$'é?¯yBlÅ4FGL J0838.4-3952¿Ýø¡ª'ÃÅ?ë»'ˆÛuÀ9yo/bÄÀ:Ó¥á¦x¥@˜é6ºÒ#@ÿ^Ö?ۺϟ:~?ãqbx›Q@jl»=¥@"©ë¡ND¿àq¶ùê¿Ü&n¿%oP¿ë²ÑCT§¿ìÕwácà¿ïûJ>³‡?ïë/=Û,âUNASNone?ÕÊTŸ)?ÄÅÚ*Ò+l?Á G=˜h¦?» æèiá?àÒÄ/‹–B?ÈΩ†?̖˜O"ª?ʨƒhóëÙ?ÃYg¬2?ąÐz#ô²?ä©—ÒLI?Ît¦Ø§Â?ÏÔ2­"N??­Gv<.<Ø?Å×4C6Ù?¦°n5áÊ?â•&Cé¶-?±
÷ՔÎ{?´Vù‹n ú?Ÿ©9küyº?»?‡äh+?®S3D^8¨?ê
>]•žÛ?±M§æò"Y4FGL J0838.5+4013?æ|÷ȁ—"@Bt# –x}À;žU9xÃÀ<Ò³‰.èK@"Ztâ*,#?ûA*ØÞ©?ÆʙÁ²'d¿—…ã{²Jb?Òr>¡ÑL?òh_ōh^¿ïÿÿ" 5•?ïÿnªØ†>¿«2Zp8ø¿åÍ}å¿ØÊE¾¦ƒ?ѳžþ]h'UNASNone?琉éJó9?Š[Rì€Wy?B¶ïŠSs?AП×›?"ñV´ž?Š£ZÛå?îpr
"?¥Æ±¿Ï?u#,ô/è?'AÀÇ*?¦WÄz@ ¶?£¼{
Äʤ?í¥³ýÑO?"
@æ›Q?'ÁÇ óö?x-–÷j²Ü?°'؃§
?'AŠ™øt®?ê_…Ì"#B?¬ÕM¤ÕÛ¡?"ë@Эã?Ž—èRK$?Ä€³™Ï€?­kl"'VÛ4FGL J0838.8-4552c?ê­TƒÝ<(À©Ðé'ÿqÀ9]U÷ƒY¼À:2`Nq@ o]µ<ã5@—¿|'1ž?ß'kŸ
qÉ?ìÃ-±@`Æu(@qÕÛ>U¿Ôºªö¹/a?ê_ä¡Õ¨>¿êvåں̿ãá"ßþع¿èEÓI¿ïÿÙÔóüUNASNone0?Œ»Dc?®üÀ
÷?¡aG4Ý1¶?«":´?îyԟ¡ÜÌ?´éy!SZü?³­+Ér)?³ÿÃƘn¥?¼ÔÃ}µÅÇ?Á–PF ?éïÃÊÐ?Âö"b­À¬?ÇƦB"Áu?¥ØI%õ§^?ŘO¾%è?§Õ')­4?ä¨Bíï)?­p…mý)€?Š‹åfŠ ?{DÞØr?¨à¬ þËá?¤šÎkñÍ?îÅ W©?¥	k#›Ê4FGL J0838.9-2502¿íÀfÔd4¢@#¿¸jßÀ:ˆ[3,}7À<GĐ¾(Å@æ)ÊÔ¥@ºñ¾Ýa?ÒϏìTR?Ùz®ƒ?ýçdã¯ga?õL®Cõ£0?ïøbaô瞿àpLÎå«Á¿éí{˜ý'g¿è%LÀ¢ó¿ì'¬Óª7?ÖÅ|vs#äUNASNone?Ûàא`ü–?Çl_æÕî?³hݚDáú?±Y|X°+Ã?ßDñ	
Êì?ÈÅvÖT+z?×VCÈ£?Ð
Š<Höî?ÐçW¸?ÉÉ$;»á?؎Õ2£¤å?̳6dUé?äMˆÿ3j?¬oèðVÒ?¼=«§mœ?ž‹—A˜th?ÐUƒѐ"?§@ùþn?ÑÄVFQ²†?°k‡½¤No?ÚÅÚTZW¢?¼neŽÏo•?ÓuÏeSõØ?¸FNÏA2ã4FGL J0839.1-4613c?ãÚ¾§ðõKÀ>‰¨‹À9q ٔ[lÀ:ªi³øÀq@ ¤ù9@FE^¯?Í'ØŠE>?ËHoÛZ.J?öñ§ãxu?ùSj…ÚÊç¿îcϝ·‹r¿ì "@º?î፞¹"¿æäW}•W¿æãyÌz¿êøsCÄ{UNASNone3FGL J0838.1-4615$?ŸV»ÒOÞÍ?˜HÚà¾Þ0?†® Ð7?ŒäòiI=?î­'hê@ú?ž÷*gå¢?Ìö0'+¬#?ŝ©ÿû5H?ÀËõǜß?š'™‰öòG?èCp«Ýö"?ÅH>FÓpG?Æ ½2TZ?£è;WˆÃ?ºÏОí"? ;G˜+‹(?ç%½¼òÍF?§çô:ø
?°^¬ÿ·ä?¡«° Â?'€Õ8¸ª?'Ĭâèm?íh#¶Wˆ^?¥æ´.¥?»4FGL J0840.3-4544?éÒ¹Ë4¾›Àp²˜À:±èkŽÄTÀ;ºB<»r1@#'½@è¨u?ý(&¶Â?É£{æÖ¿—çÁ<BGð?Ñ3¢÷¼:@ŠF~¾w¿Û¢<€cé¿ïùÔØ4	?ïgÖs>»ý¿àÔ&~ïʿ嘑AƒÍ¿¥µna\'PUNASNone?á%'¸‰Ñª?ÆG›ì=À?ZùøËñ÷?U;×±f2?ݚ– j´?Æ…@Mð?Ñ°gãí¤?ËmûxW†7?ko^*]l?"ÑwËõ±?çPíã«Ã?ËEYþwŸ"?â×ctŠl$?¯ý¡p@Ž?š—w"#é?'A
B?اÁ¨é'?®Åé_,ò?Úi¿³Eû?»wD!2?z=ÄýÉ1?}ÐÙ8mêä?âÊO–*Ê ?»P•]x
…4FGL J0840.6-3130¿×›Ø)_å@3Ð9h×ZÀ;Ué'9YÀ<ׁ›v¬@'1È$@ü.Êî¦?ÖÜAÿÿª?íøЁZ@ñ¯:ÎÄ@
$ùS¿ïþÊá:B?ïXÛch…?ݼ"C¿‹¿èÐMUhÇ¿ïÿôÕ÷?îb¿è¸¼UNASNone?׺B×Â?Ãõ}ìí?Õ'Éú£ª?Ä­ûÊrö?ÓÃ"U"?ÃG˜Ê?ÏÝ2šq"?ËdA»/^?ص\U ‹Â?Ïfr¢X'‰?×\
]Ü»}?Íy•Ý<<?Ý>iKR>'?²åíGQ˜?ÒO͒½T?³‰[üç,°?ЮFç?§½f1¬×?Û²`«;J\?¼ÔlµC8™?Ü2+Eé­?À £øþ…?ÀhÚRý—ì?­H· q×4FGL J0844.1-4330?èr-dÅ°¿àíQÂjs;À9Zox]߯À:š‡–ü@Ãay@ y½[?Â?ÎàÀʊþ?ڂZbÌþÌ@
RÈ>Ȓ«?ûæ"KÑ吿ºÐûۃ¿ëéz'}¿ãÌôÀ0Ý¿í:­³N¡¿ïÿ~Ù#ó¿ïûR¼ev|UNASNone1FGL J0845.5-4327c?Àº¼>?¶¼±›ºG¯?§mÓ(u'=?¥¬¬–ú?êZ^rWh?»üÿÜÎ ?²´IÒQR3?±]Š9ØS?°Xu
Ö?°í'Z;îÂ?먷"?µç§ çvS?œø¸ÿh?¡Àk?»ÒÀ?ÃKPŸL?¡Z»2f0Í?æ…þ½Ó­!?¨F±8-?"¬]¤õۏ?³ÖÆ?ª?¶5›WM8?¡xZš¼s}?ì"鯍g}?£¤,Œ¯ã¡4FGL J0844.2-4554c?×tö")¿ÿùyÔttÀ9N:¶~­À:³>Áï-@"#êÀӚ@
KáQ?ÏFªâ?уZ{w?ý«·ùÖñ?þQvg]?îyÞon¿å<5œ}z¿æe墆¨%¿çœ&;Ó륿åéÀ°3å¿ïÿî,˜å?UNASNone3FGL J0843.1-4546,?²ª0ba¶Û?¤ÑŠ(pyE?‹ÏÍ®Ù[Ÿ?†
MH±?í;z¼øc¶?§‹°¾¶0Ó?ÁÅ
¼ØäD?¸¬üýÜÿÕ?™'/…ÊoP?žcæ~ä{?êŃԛsu?¹ïÉE?ÅjXˆÂlÁ?¢–9àN)?½+IøÐß?ãçØg?çžµHð?§vâþ3²m?ªÔ߬«u?'Ïg¾¦0½?¡&ñã44?ˆ!¦'Ï?í@Bçò?—û$Rw94FGL J0844.9-4117¿æP¦•Dd"?ï l¡éÊ4À8ôÃóà7
À:ËeCP·¨@¤d[Ÿ8@±a£Êu?ÁSŒÄôç?Ò`…_@V=>Nð(@Qï x¯?ïÚ¨W¢~E¿Ú"uá-¬á¿éÃ}Ò霿èØRq¼Û¾¿ïÿÿ>¹ú?í쉖WZUNASNone?Ó{çNFQ{?Âÿ՞ÒÕ4?Æê­Åt­$?½H.\3…¶?à‡`ç«ú?Æ´þ¸õU?Á:›l¼3€?Âà¶70Èú?ÆJ€ESJ`?ÄŒ…ßñÚ?æ¹| ˆ?ʊ!'ßÐÍ?Èý¦Úø?¦U]?Ìec‰ÿT?©0é
?âö'=fÿ-?­OórØ?­£#hq?" >='L?ÊÍÔ¬¿
m?°k¢Ù(o›?ç|`¢™³ž?±ö§Á¯p
4FGL J0846.6-4747¿ï?[…6áÀ½g\/«¿À:€vÙ{0ùÀ;¢&äpX@!	¬&9%@|Ą(ï
?Â"O5G_¿µÅ3{W3?ó²"ý[
@T€œGžÐ¿èei|Æ¿éƪß<;¿êúŽÜ§5d¿Ù}®A~6¿äCt~­0¿Ü.Ë$V žUNASNone?ÚHÃ^!?ǛËß&ßÐ?¢^Ü.LB?íw{[?✲`¼tX?ÇÉAÔa<?Ñ¿×ÅU³E?ÄšMxD³?v‡íá?Žä,	ÿ?æóîRò?ÃÛãŒú#Ç?àº8ÉoÏÊ?±oâ[°ü?žÈÕÉì?ƒéš\?Ü¢Œð"Í?°Ëj{o±|?Ö4(iv©?µlܑgQd?…=ÁÐ1?€IÛÃgzú?䑚Ô>t??µ½±ü=ö+4FGL J0847.1-5954?ïý‹x'¿À$••ÝLvÑÀ;cÉ
ûkFÀ< ë'+@!Ù0*Pš?ý«¤C@Çp?Ï-=û¹o?­Çƒêó:?âéóN@Ö?ÿ6±Ú~?»Ò6T/=¿íê͈ê?®%CÜMÉ7¿à¼{Eñ|¿æ¨ÊYUì?ÑÞÖO,þUNASNone?ìÄ8z`ñ?¶Šü2ù?BÌHj
PÁ?>X¤|N…?¹¸£œ$c?¶LÒN…4?ã]°ú÷ߪ?ËpO¯²í?này1Õî?'iý»Ú@x?ÙÝåÝ?ËNgnFæ?ëèœtB´W?¡Š–©€‰?5J§±½ž?lù€e:úÍ?¾ÇdzoAq? §Ï_T_?ê+ZlžS?¬–‰~ڀ^?},^­~æÒ?uǨ
¼?Æi3X¼¬?­Åü1p4FGL J0848.2-4527?Òs&#'f¿ò´óý">6À9OðøûÿÀÀ:ÚßVø4@a±U¢ô·@C›0r?ÁM P+?» 'ÛŠ?Ò2ÚÞ2zÒ@ìIڔ‹"¿îƒ¿<ÁQo?ïéªS%A¿ç¿6ÁÞ[¿ãâ¾°ÕJ¿ê28A:
¿À\Þ'h#ÖUNASNone3FGL J0848.2-4524?Òé¸háH?Â:ø¨Jð?²X¨jë¤?«*/6bgÕ?ä@#C>1ç?ÄIloÐ?ÔDE:""Å?ƚÜnº¾?"TÀ7gb?"ðjÔ&|?匊aà`?Æk·ç}æ?Æ?ßd…	?¤¤3Ææ?¶ùž»']|?šXe‹U?çÔOl'?¨}o~?Øq3¯J/ß?²'÷Óϑ?£¬²ü}ó?X¤4¯€H?â•{]+ 1?²Éªàl•4FGL J0848.8-4328?ï]üûœL?Äñ€uÜ%/À8UëºÎ‡À:aŸ®†¨@ƒv‹w—ç@OÅÛAÖ?Áh™ Öd?Ã[#§¤õ@K#@¬	YBg?ïÃ>Ò£¦?â®
ŸOæó¿ê0dKÙó&¿ê†Âùå¿æ¦òèÀHZ¿âÌø6#
UNASNone2FGL J0848.7-4324?Ã2&ŸjD?ºjKqÚë?ºPAéO¸?½[£öÌF?çévy.3y?Ɔ‰îçcq?µ,±¯:?·!1¹"7×?Ì0ñ"Uf?ȄäOaK_?æN-ƒøç¿?Ê—ô×%§?¿K¶úÈé?¡)"þ	Æ?Áv2GJüH?©'ªNÐsÝ?ç¹7MçÑ?­§Ž³‰±'?µ:ٝ^?˜¿gVÉûB?Ï Ž&\°Ø?²–úàæÔ^?吁Fu'ù?²í¬ÒŸ‹‹4FGL J0849.0-2702?ëýt
•e@$óÛYXÀ:¡µÿ*íêÀ<*hþÇÜ@)=Úù@v»cýM?ÍZ÷¾=?Éë9ÊQ}?ú¡:wË@ÙùŒÉQ˜?ïûÜpêN¿ç©µ2&¿é/ýS}U–¿å7ÖeÒ°¿ïÿt¿Å}M?ÙÈÞÁ
XUNASNone?íŸÑ±;®a?¯
¸l$å?ŽW48'ä»?'VcÃXÌ-?®mÞ$`½?«§A§³.Š?éìJÊ68?Ź—%Ì­†?"‡–+f"Ž? kăä_?ŽâºK9?ČI¿èØr?êh$ýxÏ?¤Š%ÐæD?¡†åQ§ÅÈ?ŽTŸWòr?ÁýÞ +T?¡výÝæ?쉿(A{?™üÃt™?–ÇÖÜ'ÛU?'»Î\z$?¶›ýN?•Å÷€%‹4FGL J0849.2-4410c?íx'àÅ}"¿Ìl‡g½ÔaÀ9ŽËŠ­mŒÀ:ž¾®üØ-@Èíº@òâÆ3U˜?Ú®4Ã?©újꯋÉ?âÁ@Âgîý?ò²jž.~Ã?æ¤ðzPþö?ã²ç®6¿æ]Ç[sÄ¿ìÏÿ‡4<H¿¢Æ¾bHA¿ê\›A9†4UNASNone8?ÇÇ+%–'?ÀE¯8g¶Q?¦	¡IN'\?­¢¯&SZ?譛"–Ë?ÂɋXu~õ?¶ôp"¢H'?·_œa(éä?'²6FÞB? ª¶=B?ì"à=4ÆN?¸s®p4>?ÆJ€&îç?£}¸ÄW'ˆ?¸x÷¹ßh?ŸR
°ª'œ?ç^xÀÿY?§|$û¾•{?¼)ÃÈoÙç?§…Êp̆?†Ïzã¬(Â?ˆ¾þ8Já?쉛cT ?¨àH=hg'4FGL J0849.5+2710¿ïé=nÿ½@B`'ݽµÙÀ;:I¥ÒÀ<š…&E'@Ɖˆ*@ þG™Å?Ñd}£Cç`?ÊÙ'#0?öS¡Qô¿@ˆ3û°'¿ïö
~C›?ï•Z0Fð¿èªq"'¿çq'úä¿ëK»%_5¿ïÒŽXUNASNone?î3ÐX_N?Ÿ'òc¯à?ziVøb/?uâì¼Zño?£¿˜xžÖ?•^~tÍd?ï4ðÛù›?•Ò·ÎÔç¯?bM
†äkñ?qìI!¤
Å?—C0_H?"Yôěæ?í4´×hõX?˜iB=ã",?"ÄØE‡?ƒõ<0'?±y觗?"þ¾7Ž?î£ô蘩)?‡Ãs[‰î?'­¯Þg.µ?qâU'‡?¡E~Û¡Å?…lÎn˜K°4FGL J0850.8-4239?êï:@	? ¯ø×À8È.¤X9}À:OfµN+@ÿ¬)Ü@	}î$nt?Í(+Zå?è}´'l¤@«y"O¶?ù²¬Ñ~¿Øs©ÏqÿÙ'{#â³>¿í*¶W?ö¿ï¬¦Q8ø¿Ý©y¡Á¿ïçÑ­ÝUNASNone3FGL J0851.4-4244?¨5çË?¯\潤ù<?•HeÈè?Ÿ[á€!?íÒ^`'V?³õø7­xc?¨k'·á;å?³*»Çä‰?Ñ<[U<y?ËŽÖ9qN?åÛ)ãé?Êòè(óå?Äs}Ÿ£	)?¨º"Nƒm?Âʏ$^?¥Mß2OŽf?æ^­ôN9?°[u)|Ȟ?oW'XG†?aôå´¼£?ÛM‡ó&͜?ÃÝíDҚg?â9ätí@ì?ÃÉ'
'4FGL J0853.1-4407?æ2<	4uí?ֆsa¡…¡À9pNŽÙL7À:ž¢¶xÍq@åÿjþ@Œf«/Ä?Ð%lZþ?áf¦ÈVE‡@ÑÓ¾X•Ã?ÿbÄî‡Å¿èØ?ò‰J¿³ÓÿÆõw¿æ%"CïC¿ì(¬A<
r¿ïÿ|¢gô[?îÜ'éSQUNASNone3FGL J0854.4-4404?¾Z¬3Ñj?³gÑf•"?Ä>"Ñã%?½Î=Ëô
®?ç3šÔ'e	?¨Õàa£?»mNpØj§?¿½H¨öÔ?ÀÔ&mE?ÁZƒÓŠVY?è]R0ÛWZ?Æ@û‹!P®?Ã
ÁÎ<ó?¢é,ƒ?Í"N^èÒç?«yx<*ð?ãóüR<	?°%hJT]Ó?›RW…Á2²?ˆò5ï"³
?À+
°,f?ª5Âsü‰g?ë©×ÎkQ?¬aCut%ã4FGL J0853.6-4306?ïä¦i¥yæ?ñ%ð¥)À9
OH<¯´À:'²jJ÷@RÎؕ­Ò@ʁ~áS?Éj )?åÂ:¢"=@I!ßyx?ôIYˆ²l?›ƒi+'«¿ÖO'Ÿ,*«¿èeàš	+"¿îÞ§ msK¿æ©n)©G¿ïù>/GìUNASNone?É(ÆþÏ	â?ÁöKÁL;Á?Ï,¢0õuÏ?Å¢lÃsz"?áꥴà?Ê|ÓÜñ+A?™îSTÏ?¤o·<ÍÉt?ÍÀÇPד?Èü–Æã·?çÀ[¢Ñ#£?Ȉ{|
(?ÁSb™÷²ž?¥'¤ô¤?Ϟås4¥É?¯Mtd
å?ãÃmü´éæ?±ºÌRªE?dóîkÔÉæ?Rlÿ½Éh?×Yhô+«?»šØáH²Û?ädß]`?»œÚÜ´L4FGL J0853.9-5501¿ï¨Å¨ZÀ!º^5?}À:¡îM¯À<
'Á8D@ºSç2Ԕ@þtYœT?Щ•$¿Òé?Ñ*¢ëÒÌ?üíV•8	@ƒt¿±?îûa3v¥¿áÖ!_K?¿äK›^ëÈ¿ç&#€7ÈĿ런9F¿ïöI"]ÍæUNASNone?β(ZÑö?ºg¿×緌?ž86f:/Ù?"PPÎÍþF?ça´6êD?¼&òi6P?ÑMI
ð?Â5dI?‹ÒÊn~g?"6l…fÙK?æêQBb?ÂMŽÊ¤Š?ã5Â5?¬M‡[?¸@ÔC<å?šø¼£u¸ä?ÒÏ_kÝ?§¢±ïˆ8ê?à~'}cI?©ŽíCÜ\?ªeÎ­Z?'–'œšT?ܚÖ,ËcÅ?©p»a4FGL J0854.8-4504¿Â.ù°¹#€¿¡MŸßȖÌÀ8"Š'¾ÙÅÀ;H"ÅõB7@üíåKHÔ@
™#R ?´7¬"ž=?Ý/0ÓÊ@#ƒn—?üL+ín­Þ?êñ"¢A]î¿Û£iüóÜ¿Ê÷Ÿnc‹¿ã´k!a#±¿í]¶>•çÞ¿ïÿ³^¼£àUNASNone3FGL J0854.8-4503?lwW½EŸ?i­Mù…]b?í£
§®yç?°
þì!B?²Ø¢Ó?¯b{9À‹?yó މ¡[?'­O¡ìú¤?è«G58×é?Âmïùc?̃J$(SP?ÂRNé.r½?ŒAȚ÷?|ÓX^šT?ìUB‡á#­? me­ 9?¹Í²­˜X?ž}u¤z1À?eg—¼E?MˆØ¥LÕ¬?è2\H>è?¬Œ×S:ý?Îâ/ÔK?¬oɚ	Ú°4FGL J0855.0+0720?â»tŸ±ƒ@>Åé\îÀ:Ã<«ùjÀ<\R±}»î@
´t:å@¹™Üµx?Èx/çyKp?‹Ì*IP?¾)lµàÍ
@ԆλºV¿Ìєݝ)œ¿è|u éY ¿ç[i³"¿çêï͂Õ2¿íÁ¶ÿ0![¿ïÿï9_JUNASNone?îü¨bÑ?šoè}É?–?y"¤GdÒ?|°@º+Èn?—®2Á˜ól?—™j€ùþ?ï8K8;(?"Oðª mÖ?_[\ÄáR?júýûpõ?—§Ã,Lò?'šìíØñ7?íyñÜà?"âüÞèèç?ŒC?Uå;Ý?{Mñ¹Þï?°¨	.>ԃ?'ø/°u?îúpRŸpÊ?'[æL«´9?|ËsýÇ9?i]Jʦš?™¬ /?€…°½1H4FGL J0855.0-6026?àa*•ˆp…À#µKjaªÀ:Ï,?#+~À<U™OǾp@Xš]¹Ä‡@ôº¼ÿÐ/?ÏGRúν¾?Ñ*ò‡qxé?ÿV­ÜF½T?ÿt'Ln¿èã'Á¹m?í£†ŒG!¿Ü~óûå¿¿âò(؇¿éÔÈ¿L½¿ïùé€aº/UNASNone?äƒ\Ò
É?Ãê°
Q?˜dÓAË|?'{€­ž+?Õrù'ɇ?Ê9‡+?åÜ\xKx?Éä6#óò?G…ð3íÖ?"{kô|'?Ó]
à?É¢?ɕ음i'?ç°K¾½O4?«sSF~Õ?¯OÃ1Ï
 ?•?úY¥€?Éjà8—†?¦¹°,×W?é|«£ˆÓ? $¥ü½Wj?«­Íï=ê$?'1â?Îa?Ã!Ýöf(?œjyW&òÅ4FGL J0857.0-4353c?ޚxÈyè
?ð'Ú:s™UÀ95–4ŠKHÀ:}NÏpëû@¿ÃJB~@6&}BJþ?Ò#1=9ÇL?Õ¶¥ä*·d@۔XÖ[?üo|½?æö?ìåÁX¨8¿×"›¾7Ô¿æ"Mºö ¿íG¨€gC†¿æ4óý">6¿ïÿ
Çhß½UNASNone1FGL J0857.7-4345<?ÒÄiüÜýú?Ä9Š'y"ì?À¤8v°Ð®?À)!:!õî?ât¼ãåL×?É`µ•"ñD?¢/Þïå³Ò?¤>ÌA¤?´dMb4â§?µø'<{J?ìPxd»n?·ì&ºVÀ?ÁvX
ôA}? \»È¯~1?Ä>š?§ù2ók\?æ¡ÚUÜi`?­f¿?Ž4¬ÿÏ?sé`¸Ô?¼pÇ-Ã=?¦I|¿"÷?ëùf_ëR?¦B¡ÓœP4FGL J0857.7-4507¿ßpà¢â‡?Ôð°lCõùÀ9_É'%Þ·À:¯"¡@ÿi«kG@%³Æk‰¼?ÍÙB¼h%®?­N—½¡a?ýäJ|ûÔ!?þ`Z³«¿äý ¿¨¡õ?ï
}—"ã¿ëfx¿âyì?®ÁŸ¿î–#ùŒ|¿ïÃOÀ²0UNASNone?²5çõõ&?¨àõ(s?°ÙO
#T?±Á}ÁÙ?ë¤aÀ<ò?·´!)5N?°ú_¶ŽÑ?±]'ߜ?¹c ½Š­f?»"ûÓ(Ë?ê´Oñ‹¸y?Àt¢—=¦	?Æ1¸Qß?¤,+	µàg?¼Ç.•Š~j?žÐ
9ڋ?æÚ¬
xs?©ª<:?µ—¬5q^?š_ w—Cl?¸Å$Œ;¶?¢MÏÃñ)?ê4xò'Ê]?§z†îÝûû4FGL J0859.2-4729¿ã×:@š¿ðn*¦€2À8ŒÓa;";À:'
—~6@&®¥Ô@Âä›ök,?¶À:Çý?ÅÍÛÕÿ%@
èþüÊÁZ@ße»Æ•?ìäÀ™+¶¿ÚŠžc˜V¿æŠâ¡ö4z¿çì2"'û@¿é"¤!²Ø/¿ëbZ¾ž
UNASNone3FGL J0859.3-4732?«›ýu£\?«›†
i—?ÐUiíà
?Âu+R£¨M?æ¼ù!µÃ?ãšH8?­0U÷ÍÝÿ?¥	Y°?¸¤;0‹ô?´E'®MÖ?ës:q±á?·EL´%†?Á¿Mžš?¢Ù꾕R?Ã¥¦"Gd?¥CÂŜ†?æ¦ÕIOê€?«4CðNë?¡¨úl³o?…€²fäÀ?ÁØ(€ôp? ùgfîª?êx›PÄ?£`h¹"é4FGL J0859.3-4342?×-rKn`?÷]qËväÀ8¤ç2© xÀ:Š·y¥@‡BÈÒlI@쭀k`?»@|`½sØ?عïºãkJ@9#'Õ?ö‡ÌbCÁ÷?å°8!Y–õ¿ß|÷7¢L¿ç\ž ¼ã÷¿êWÕÿïýÄòã¸?Уi&4G/UNASNone?¥k­%gøË?£\Ánþ5?èØ;Ù
?ÄuVGÑ¿²?ÇD%R1Ś?Âá9ú¢pP?'rìì
˜?›À¥"dž‡?ÜÊéÄPw?εá'*tˆ?áóѼßX?Îf3Wàgõ?±ã$A8Í?êö'37Y?ä·<>óH?¶™=3ñt€?ÒÄzáË;?²ëg"×<z?c1'÷57?O¡wU$?à[¨‡þ?´²:휫?ß æ…ê‡?´§jt!Kç4FGL J0859.8+0053¿Ï—¥»2gÿ@<®Ü]cˆfÀ;9!‰½"À<¸d(ž"»@"¢ªÜâïy?Ô*"}ÙI³?íEÝYâÊ?ïÿÕ7ÕYc@žÁÁÖυ@B)"â?ì»m߁…Q¿Ó–Ñþèk¿ïÿ4Þ®÷z?ïñ
žÏ
š?Ù·`9{¢¿ãÊ?wåUNASNone?î?Nu`\0?©QÀàJXÃ?˜Î\|®*?™^ž›Xz1?ŸGÔ×FOp?£)3`ÅÌ?î'ÝÛ ‰)?³²'}:"f?~"¹@¶a?˜BuÓ$xü?¤ ¶ÏV ?±PWrÝÎ?ìJôåŒìï?¡Ågq§ö?'ò¢*9óÕ?ƒÉH6ü5‡?¸ë°I
—? CÜ÷Àß?í"ó'›2?²+_`?CòÑGIWA?y2·œ¬Ì?·{rÀ䓹?²BÁOúI4FGL J0859.8-4530c¿ë®ÇÃoù/?Öù¾'BÀ9.Ž'uÏÀ:§†S€@O›æ¥ç@¸1ôo?ÔùAÀÖÌ?î¨Ä_@x@£ßm¹@ÿ?þN>&I¿Ê"ù#—ß°¿ÅuB⨬1¿ígß7]¿çڙz"¿×¼Zcα~¿ïûï¯OäUNASNone1?µ"ÆÁ?±"45Ÿÿ?Êkpû²…?ÅèO»<lé?沊ÿQ!¾?ÈGÀ½i¨?ºÛBÝõß=?¿|™i^"?ȊƒÎCù®?É(æ{.
?æö°°E­?Ì¡KòÚ?Ë¥Uù"€?¨—3WØ¥Ø?Å`[4&^Ý?ªŸö³Þ|U?ãá¿Ýx¨?°«òš=?¡3ùÈ]B?"z6¦ˆÜÓ?ÍÃaÆcڜ?ÂÉ°÷?ç{çñå#…?Ã%·š4FGL J0900.2-4608¿ïÿºÄÑDš¿†* Û[ À:Ž‹µ«HÀ<hõŒßw@a~#òM@'ª\_|g?Ò|Jž‰Ãc?æüÑA¦"}@	âšÛ¸ù?þUºêw,²¿èÌâÑñϼ¿å¿SÒå낿ӷè99Ýq¿åÇ¢'¿î2ÜÌQ¿ïÿ'Þt†UNASNone
?ºé¦R&p'?°HÉä6L‰?Ò\nûԓº?ÄV¡ÝÄæâ?ãt"·Ðè?Åt=yæ?¬=uC%&?­rr–bŒ?³¾Q¾F7?¶%Böt\?ëÆAðãÍ?¹Ž˜v¤D?ۆAÉ«A?°ÊT D&?ËÌ mbX%?¬78cË&Ž?֓­ÿ£Í­?¬Wc+,e?½Ô]|ð³?¢½$üû:ù?ØNOhÜá=?º[üÄÖó?àLœ'K?ºéƒ'¨p4FGL J0902.5-4727¿ÔJNd´W¿âŒ0êÄ/À9—áZùJÚÀ:Ëu$oK@ =¢wä"@U
`¬B?ÆíÂ;?…Õ£òQ5?ÄøŸ£ô¼U@ÅKSuÙ¿íék¾êáá?ïî5gÀÙz¿èQˆ˜`´¿é5#˜‹| ¿á§a8)<9¿ÛoÑ~ã4îUNASNone1FGL J0902.5-4731c?ÆxˆQvBö?¹M´ù#?—''–^â³?—T(ë"º?é¥I^ïx-?»?*©&@¶?Ç^«Æ²×s?Ã¥d2ÿ?~üÜG†e
?Km3^?éê[UÄ=Z?ÀŅ*z?Æ|{2ö+?£¯_={IP?´âÚdÎÉ?šk}â²E
?çÄ¢Ô²Hœ?§µˆ.ª"?Ӟ%ÅfÇN?±"Ì'šj?‡Ì™°ð¶Z?y"å²í8S?åѺ¶ˆÙ?±°$23$Ë4FGL J0903.5+4057?ÑÂz_¼@DÚË}At?À;­RÜEæ"À=û¼¤`@ {åóìÌ?û¾Îø 7®?޼ɴêWø?ÆÂx¡[?íìw¢xæF@â!Üɚ¿ïÿ€H»Ê?ïõæ °Ï–¿ã¡Çe"¿¿Ø»;ÀJˆd¿Ñ5¡l犿ðUNASNone?ïÄpɇcA?ü1Ì¢ 7?OnÉ.!áž?P³j¶Ñs¤?yÙŠ#F?€ý–q¨??ïŸýAö°?…ÇËr{®[??ûõ}'%?R@–C*gG?‡Ï֓JÔ?"ÁAœ?í¡B&ÕHš?™X‰þû•¹?yâÃÕB‡¾?mS—öWÍp?±WŒ'²?˜vš
Ou?ïŽÝ7ß?x'öƒ?Iþ6Ô]?K5´zUî?Ž|—çT¢?x@Ո¶M4FGL J0904.6+5200¿î²°%]@D§<`ŸÀ;X*CbÀ<Â?Úác@?o¾Â@ÚCä'?ÊÇãÍ¿¡6rWá=r?Õ[¥BDH@
ûx¹ u?ïõõòðM¿éÑ(| ¿àœúAzÓ¿î›;ùç¿ïÐlÊ-¶?ïÎèӓUNASNone?ïé
ÈB_?'[~d}÷™?*ëŠT¸¸N?@îêk8Ó?dÄ9'r
?§þ>@œ÷?îÙ_4³Ö?«:e/•0?dsUãá×û?vXÎòô"@?¡"ÙÞv¥?ª‰‹·?íõKà]ªñ?–q7ÈÓ?'$ò'Þå?|³¾óÅáw?¬"t›Y;?"ïÞ*t?ï¢3£tv´?t¯Œ­¼?R¥|Æii?JÞjùI?…gŠ %š?sìX#¦¾"4FGL J0906.1-1011?ëæåÛD@7ä=F²køÀ;ÙÙ$ÉäÀ<­¶‡*@üÎí¹Vx@Vçæ-Æã?ÇyåHn¯?¥³Ûd?D¹?àE†6`å?ñ¸'Æ@Á'?ïÿWߣ¿êw?&±p¿á"g¾U:Å¿âvYޘ§+¿æx²™Dà?™ü%]1šUNASNone?îÙÆM¥ö3?ŸŠ=a»"ß?Wõu±Çuu?Tû'Št"Î?¡£ïxa,?žîø,ÚïÓ?ìRß۝—?¹+Ìñ?•\ 5ª?£fQH¢è??¸ù[Õá?µ€ì4·ô?퍨úдb?–&ìàØ&?[OæzÕ1?tY²°÷ª?±gN,«F?"ÆXè?--?瞑ŽëëÅ?¨z÷jTд?©<¢fÍe?•'[Ö.çJ?Ë6'*?¨^´<îôY4FGL J0906.2-5337¿ï÷o{kŽÍÀ"?Åè­À;ƒÉØ)øÀ<žæs.Ì@#XîßFL?ärÈ^þèÿ?ôP|V?ïõJšX{@["UU@ӌ1Q0Ê¿ïþÜêQB?ï˜Ê õîÚ¿ð?ïÿÿ&¦³?êbÙHÜä¿àC ´UNASNone?éLĦy?Ȩ­Öudq?eöï¶? *7¡ßÑõ?ɾK§=²?È?Åæ82?ⳤ??ß?ÒÚh«u2
?…à#
n*?ª¹loÞؚ?Ùðˆ€gî?Òfe±†?é®Õѧx
?¥¿†Ôwe?šÜŒ¡È-?ŠÅvs›TÏ?Åé%)$?£ÕÉ¿¾'—?7È
Ö?¥ÊÁ¾|ÿâ?1y'¼þ?qTÊä3Œò?¥£øþy¨¦?¥¬%Iœ4FGL J0906.8-2122¿èŸCYÆðÀ@1.¿üÚ±'À:'ŏÁªÀ<NÐ& û@F»Å™5@ÎC$Aþ¨?Ä°uh·Ïe?ﶰËåF@@Vý<×!?ýÐ$ˆu…¿Øå#»qп±áêìžF¿è×Obîœj™Ñ;¿é>"Õ½6W¿ïk|»<'UNASNone?°QWÈ$…°?±Õ"tÑ~]?맯·2µL?¾"8+Gæ?²q*~EÏô?³ªø-ç?'1VÓîy?¡o0!Ü
?î#ü?zC?°ßÞ
ϑú?¤§'
d–?¥÷¹¡ì´5?Óc%{Ïs?²¶$½î\?ÞÙ]™|,?´ÃÉÆÞÄ]?ˆùÕ@êÁ?ªéåÊõLf?tb^9ǙR?o|¼%š]±?î×Ѝ	B?Ÿ5rÆlP¥?¤–7/öxÍ?œBê¾4FGL J0910.1-1816¿ÎöÿlB"›@3¿.Y¯ž¿À;)t"&"À<™™'óe@ U'}‹Q?ú€3çŽ3?Õ?¹=ùµ¹?áÒáïsÁ@¦"¦óõ@N·[÷M?îÖì
µÃ¿ïûÉeeà?ï³t'Ü¿¿Ý~ŽÑ¿{¿ïømÏç3€?ïk²ÖuUNASNone?îÒÇsœš?š¥æƒÙ?…LmÕ\=C?'Ë¥ZÃ¥?›p&ÞNF?•žÈ\AžD?ì"ðr¨F
?µÞŠÂl¶?š¿XP¦¢?¥WJ9¤Ñ?´¨¦j©¥é?°´2ˆŸ•?ê`-ƒ‹Q?¥A»5øµï?©>@;M1(?"^‡BÕTt?À/¹¯†q? Þï€1 ?ék]=eø?°é­ÿ«w~?–2fZg#?'µ˜ùP«?ǍiÈ=?°I,ž¹4FGL J0910.9+6055¿ì}èU¿O6@D:Ü
²À;€Åt÷TÀ<îÈ8–@³Bâþ'?üiÇ)Ý;?Ô¥:´e?Õ¥óD/Ú¹?ÿîãª2n@·7œ¤eû?ïÿÿ^ðP`¿íõGàiaÃ?×de$œía¿ãí:`Nq¿àq9~%õ³¿ðUNASNone?ï>ñ)—?`¾½[`?Yóýî½o?YV"®Z?–œâ
ž2Ñ?œ•tFÎýO?ît.þ|Eb?¢¤‡N	<[?u—wàöØ?ƒŸ+L/?¦
!ÎÖ?ŸûGp'?ìOÊê©^?ŸÍ>ïñ^?–w:ÀÏ?"øçø9hî?·ûJå¨lÓ?šùüÈ(ù8?íhépïL©?˜<°(¡I¹?vêÓF²ÿ?oK0©sI?³J[Q/…?—Hkà@ãB4FGL J0911.6-4738c?èH'`²j?ۀWÿ|ÙÀ9
!¯éÀ:ÅËÉdc@O9k²r@V½+o"?Ñ,B]ó{7?θ3b­õ?ú|°Švæç?úr¿¨X¤?ïïwâd¹"¿ÐØ
]5»#¿ìk–@ô'ã¿ç©&¿ÝP(¿é«Þ…_?Šú)"ç8'UNASNone%?ÓÓ?UJ'?Åõ×Çÿy?´×šP?´*Wu%"?ã{mоE?ǃ‡+à3¤?ÆH¿f´ŒÈ?ā&¯ªð?º(ïîôqº?½¦…€`Â?ç(²(tN˜?É8[ðÌW?È®ùGüP{?¥ç*Éáê³?ÁÓè~õ?¤íc‡o·?å_GŽ{©ã?¬—Æ9dÜ?Â.üýæ˜?¢´¦âjÚ?Å<öòˆþ?­¤5¨ó?æ%º?°¦ÜÚF4FGL J0914.5+6845?îÆÉ@	ì@BìÖÜGªÀ;ehžOÀ<ñ¼‡Û+4@! XÐ{®?÷#ք³ž?ÙúõÕÒó?Îf!‡+?ó–*C hÁ@Ãà`¨a^¿ã³!ž¶9¿êZ·D¥K¿èts¿ë<ú¿ÑUíýôâë?'Vä#'»»¿ë5tV2UNASNone?úŸÄ?ˆûËü­¤?X+¹‡H?RƔd'y?ŠKÐoL?†úoU'Pµ?ïn»äõä¾?',ýV;j?L¸àÏÖAJ?d-˜†e1`?'B¼ZĶ??×¤'ÀϞ?íMÓV‰?šC{£À?€Ðü;¯Ÿ<?tPðì¦	û?³wGÈgWÍ?™lI®S?ï*N,Ý?…˜ž¼ ?=ã¢2¼?A·TIÀ5)?šIw§²7‹?"ñð¬9;24FGL J0916.9+7756¿ìxö‹Y‡R@@åñà'Œ7À;ž«ôÌÀ=
àj8'þ@kg|×@v8äM?ËÝ
▸"¿µô<'x"ç?ækøÉ6@ͯö¨=¿ïyªæÈ÷U?ïý÷²S¤Ã¿å¼\aÕ²ú¿èL¶Ç§ÉÞ¿Ý}°6Ä¿Ð4'cšY2UNASNone?î3NÀÈÍü?ÁH}=m?"m—Îéð¡?šª3å™U?§¯­ÿ¸¤ ?ÁýˆÜæ3?ïg{ýàŠ|?6íÕ?Q0¨ì½9?cË9¹O.?'ýuµ"Üò?¤ç~áé?íDµ·'J?–$œâÇ?´ÄÁDº-?"ggA_?±­!2?+?'7'§ò?ï{~0
Õ?z$¡Ž²|?j&ąÜ_?bÏ%~i4?Š–ÂÛ£l?x†1'÷Uß4FGL J0917.9-4755?ïB´‹ô{¤?ÀIܘÀ8ôIÐ-ª]À:À4¦Ð¹Á@P'˜÷@#9¾?ǾØWðVë?ÓéÄKd­@èñƒez®@e«…ÕA¿Ô0÷б^¿á§—Sn<¿êœ…ÂL@J¿èà"¿íÁ9¿ì?û}º@¿ïÿ""ÆUNASNone?Ô>û¢žòÈ?"¤êq'ø?ɔ/e:Wü?À»Qa–š°?ÞöìªÃá:?Æu[A'n?±‡þ	??µPóÊfu?Ípn™6Tw?Ȟ"Çš?ærä˜0Iº?ÊSyž	Â?ľcٕm?£Ì¥ý.qH?Æî0mê"?¥>ëq	k?åÃ=*?«¿½ˆ;½É?°Æؗ˜?"DžYi?ђ-
Ò@3?³Ü‰
•/?åg³t?³ðveŽio4FGL J0919.3+6607¿ïþ2íN^@C¨ów[0À;$¬þÑ+×À<Ä +"I@ 5cqw'@V#£s7?ËöJŸ‹v?q$Ã-è?Ÿñvû4@ãæé¸l¿èòžm"׿à]àñFÿ™¿è@å¾5ZU¿ÎºE¡ô¿â}a?5¿ÛÂ;yRÒ5UNASNone3FGL J0919.4+6604?ï@Ú)âZ¢?µGvÒÕÍù?=‹ZxÊvZ?:J?eŸ¥?—nYсÜ?µG‰Å‡¡¼?»3tÞ?"~ôïWú?@b÷Ôq?Lˆ‹ÿ¨Ü?‹Y\óKG?ƒÝD®fO?î›÷xuº?âòKŸÛÿ?qÏ5Ým.Ë?`®í"àDÝ?¬ÌYÌÊþ|?#MV»á?ï
SàÕW?'sž«»¤…?aRɺÆO ?Qe LCRÝ?šô\LŒ‹3?'ƒ›pď4FGL J0919.5-6203¿Ý`—ûõGÀ!tBÇû¬´À;,¥R4€:À<øðž³µ@u†6:y¤?üÅ㤧?Ò
 $Ð?è1³¡'œ'@ü™˜f"@8ªÄbC¿ïþ$}㰔?ïÿ5Ÿôým?ßnD¡o¦×¿Þ!ÂÝà›a¿ïÿ胸›¿ë©ââÔ?UNASNone?Ódá^+
?Â¥G™@v?Û`˜'å³?ƪ‡Zò¤?Ñ;OyïC?Âôv¾"?Çù´Š%?Æ£î‰æ%º?ÕK«w˜?Íù)îÆýQ?ÞëÚJåCU?ΈzÑÉ?Ð/éõüã1?²A•Ñ¶Ö7?áÏ«?bo?¶ª)R|'y?Èa|}ž?§S¨@Ŝd?ßÉ*AS>?ºÿ³X§e?ØRD?4èH?¾6,"‰Ý?¿'Eýßfy?¥*QG=N:4FGL J0924.1-5202c¿èŒš5Üìç¿ój
ÃödÀ9+ú—á2µÀ;#"i†¬@9ñ–°±
@C«»Û
?Ë®™Æe)¥?¿g­Ÿq0*?ôTÿ†]|³?ô(|P]?ïúI<‰ô
¿ã1T?v¿ìˆè6ú¿ãÓW€o|¿ïØjÅp·ù?é°â`‡ÕUNASNone3FGL J0923.8-5154$?æ+TÌSÑ?ɍ)?²Ã?žOؑ7Ò7?¥r¿kƒá?ÑÄXÞDàº?ȏò7˜¾?ÑGòþ&Øø?ÌxhE"?°7ëžÒù?¶œW—ÂÛó?åUcx¹%?ÍÊ4¾v¥?×@V0Þqå?¯iÈ:U,?º•^%Ó-? £õà(ß:?á
)"Öaj?°	>)…¶^?Ñ%'
¦?´Ý£¸nÐ?ÂÎv¥1+?±.M
:p8?⹙QR­á?¼r3W š4FGL J0926.1-5336?Û"™Wª`çÀ蚈¬âÀ:"hZ\lèÀ<P+žê;s@sCC¡•?ûŽ‡Lû‹?ҏ—U»?ç€ISQ·@
ͦ‹ðd@]aXµxÈ¿ïø|}ÿà ?ÁòSD¿À©çÚð&¿×°³Ü»Ø3¿ëþYl'à¿è¡a«ÃUNASNone?Í´"døºì?¾k$¿}±&?ËvX~ßm ?¿xÆfÛá'?áµaG	õÝ?ÄðSUŠ?āÛ›t?†Ò3"?½¬æ•}¥¸?¿øÀ«íL˜?ç*'ÉÙdl?Äٓ5<˜m?ÝUTIgc?±»¢—Ìq·?Ít*"ÉE²?®íŽúŽQÁ?Ô?•šQõÄ?®#s`:,·?ᶠªVçà?¯ý7²?î?ÊÙ"°R?°έU‡?ϤA°,?«!ËøÀ	'4FGL J0928.3-2713?ç~gá³H@0úZxòZ%À;‹n]«­À<nÒæÂAY@ól¶6³E@w³•Ä"?dž<š«? ûéoð©?×=ÐE'Q~@càη]¥¿æLä_:£¿ã;¦i‹´Õ¿çš
¢ñ10¿ï÷Í⠜?ïŽÿªo«¿ïú#|ÜÊqUNASNone?ïÇ8ó–î?yk§œÄ±'?:až÷È?:.u|ð>"?z½â$:š?x·xÞÂó?îÔ`¢¼
Š?²êoÆ ÿ˜?e3å¿×¬Á?";ÊdU¿?¡f·xAܖ?²Y''xLh?íºw‹»†ð?—ø`ÆÊ®Ü?}­þÁÅc³?uêŠNPg?°Qc¶rC?–ãù¦õÂQ?ï¾íÚ0â?w^ósÉD?üØíU?ËÏâô¡?€XÇ°†¯û?wLÒÆ|Uã4FGL J0928.4-5256?Êãt)Ù©e¿ötmZvnÀ:4^'Ӄ À;²'Œ6ڈ@!ÈÝ:Ùâ@%"ü|?ÝTd0V4¿Yõp7©?¨#¹ P5*@^
›h¿ê·'ƒû£?﹞âƒÃD¿Ü5b¸[ü€¿èìí¼0¿Åօˆ?ª¿Ô¨˜¥}ÓjUNASNone3FGL J0928.3-5255?ã´½»ƒD?É[CªÀð2?n+ÒU«9?kßõÆ?ØZ,äN!†?ÉP	~2¿£?Î]Òº$ª?ÇgːeÃf?j9‡"ÞPž?'ÍÞ=‹˜?èNQØ|˜…?ÇYB:ƒ?ᐪ;ªrH?°ŽæL:Ìâ?¢q\_CÃ(?‡Ø‡]P1?ڐü£?¯ŽæÝR, ?äMˆow—?±óvp"g?ˆ÷9͔td?'ӝÚe¯?֝5SVm/?²ƒîo7û4FGL J0928.5+3916?Ú¦…1Ïþ@G:Á~ºñÀ;V›‡À<¼‰íT+Ñ@‹	ˆêË?ùÛR6-¹w?âÃ^YQªí?àyÇQc?õ
US«È@·r0É÷Z¿ë"ÿ*¿äÛibš)¿ØßüTyÕ¿ã|É´êWø¿ëáÂ]B¿ïÿž`¨·DUNASNone?³¸Òò? ‰:ŠJ¸?ƒ2 
á?¡'N¶?¢hÀ/Xª?žÃ5»Ïa?îÏ)×6OZ?¥¨ãF¿Ü?iný*6øz?~&œqÓ?¡vr¹÷šÑ?£¶GÀl¼?ëáÖmÛ£²?¡ÙSۘØÈ?¢ŒXÅ{¬ã?}´&­›?·« .eþ?œ¿7ñ=?7öÙ?'&êá©Ée?Qeu=-^"?S¥á)"'?¤"©'—'}?ë>´'"S4FGL J0929.3-4110¿ïô~¾»«×@Û¼ôèuÀ;¡}‹QÀ<šÐüÝ5Ñ@$œþ0'~?÷´¿û-2h?Òj«ûØ?£bt"Q†0?ÐXÅ>
+ã@džaƒ}£¿ï½ÜÿõÄ?ïÿí@_Á‡¿ÞÚf]­[¿œt‡Äã|ð¿Ý³n!EÊå¿v"쩃iUNASNone?ëèè§5ƒ?¾W½VÁ§?Q¦a]*•?P {
AA?À9ΨÔÌ?¾=®C5?àÁ×X>È?Ðiœ›ðP3?z
ïiZ²‡?™1ðû†Š?Þ%'Ý3?ÐDäsÝ(z?èøÝ¿"Ñ?§°¯´´?…:%ꆶï?r —æïԘ?ÊÌ*YP?§*eZX£?ç=å{ÀH"?º7¾´¬·Ú?~©´	œ¢'?~ÊçixŒ?Ñ	Ž8XüN?ºÈ‰¤žõ4FGL J0930.9-3030¿à/GÃãïÿ@.&?Ýe¡EÀ:àˆÛ—À<z á!¨@ ê
½,ñ¦?ÿ…˜Æ5?ÄPƒO*`¿z¾z~À21?»5y3'K?û1Åû!sî?ÖpÁÊoû¿ä ÜïYÀ¿åk¥€Âù¿ÖÓEA¨–ã¿Þ
`¨6j¿Ó_2•~'UNASNone?ívÓbÔæš?³%¤«]æ?b‰
»ª4Z?\4]˜_–?³µ{{y"?²ò2(QNj?ìU
@Êÿ)?»ƒ§x±^.?vù¸XÌKT?q»*ÁÈÌ?»çútB
?»°íQê­?í…ã ˞3?–Õm»tü»?zk.*Ç?hA-1ü^?²*.	p+¹?•…ö.†é?ê!|;NÂ×?¡­¶ê›iâ?Œ¡öž^*Á?z²Døx:è?ůï¨ßú?¢p¢xû·O4FGL J0931.4-3559?ïŸ%¹^A@&vT´:çÀ:ÉNÀ<\ø_»Q@  x"¦s?ú¿Íui8©?Ô¹CXr?Ò¦:&l{S?÷²åB˜@l©4:D?ïËM;5Á¿æ¾‹@hî¿Ú"Ø\¢î,¿Ýzz…\!¿ÞŒy¦Ž¿íò^ç1UNASNone?íƒY1Dƒ¿?ªXšOÖ³¡?i°\%hÅ?b›Ö ó±?³³"³®¼?©ß÷´ƒ~Ê?åÂýl(¥?È¥F¦!Í?ü8® â?Šö\ˆÉ;?ÓúÐDô1?Èa$kä?êÅ´ª{TÝ?¥×*Ç3o?šYøAŒ)?‡ÜÄßùò?ÁîMá+¤?¢ÛtßùÏ?ë‹ÛîïZÍ?œ·>ØClj?wìÅçß?j.¨à#??Á*‹\f?œElO
4FGL J0933.8-6232?ìB§øà…À¡2CI*ìÀ9þSW•éÀ<;<v¨Ô@­â˜»ù?ùï:µÞt?´=ÜÀ›ø*?æ&õ7O!¦@0M™gD²·?þ뮔¨n?ïçŸìš?¯GW™ˆ'?‡Æ¨½ÆA¿àµ¿äF¼¿îÚpžùÞ¿ïÿȽs"vUNASNone3FGL J0933.9-6232?{âV»;ô5?&kj'¶3?îíL?×ì?¨¢ÒµUö?›d`É6h?¥õäŒÙâ?{Ô¼&8N\?ˆC@P@E?ì.¨ÁA?½Àt"S†?¼Ín3"†£?½3BTIù? <|Tn?' ƒSvW<?ì>Vubß?¢'ŒQp?·¸T>Î?Ÿ°'v•r3?3;rƲZ?*Ú*1†ð?ï@»'ƒWƒ?†oúãï€Û?—œÁÉôÆ?†FåêêAµ4FGL J0934.5+7223?±1–¡Ç¯@BÏrÅz%À:Ð.ülÎÀ<–'õ@-ÄY`Ä@Œ½}¤p?Âê¹Ç·d0¿¤òåˆZ'?Û·pú¾øy@ûow‡ ¿á†XVÙ+¿æ潤:ÝL¿êžÔ6M™ç¿ê~"àÍ4Ò¿ßÜ»­?¿¿ïNŸË6öUNASNone?ïϪÛPzì?pë­ç*˜?dMäÏzO?bp7°?lʵš¼?iÚÅ&•?ïSehyç?"*Á¸1»ß?Uˆ†:Ôsø?e7Ãb²H¹?":ʙc{Ê?'Ì€

W.?î.«Ò§?uáÖ=џ?…˜£´»b?w‹Päú'Å?ª¤ìU¦µ?Œíà-?ï {…Žº?r6Æ)ï•:?j›5ò՚>?aXãÝ?TÓ¡æë?m—iìÞA"4FGL J0935.5+1152?¹t
0Ô¯@DÝ%þ—J4À;Öß3םáÀ<åCÖïe~@#^m"?ùÈÛ–ª?Ìù)a£3 ?cÕN?lì+@ÞM&yfs¿ïð®ôt±ƒ?ïìÐxR÷õ¿à5A` J¿ÖN0d¡À/¿è2D‹JK~?Õe÷áMRUNASNone?ïáZ¶æGÅ?jÎQãfLB?5>©e'Rq?XªTÉ~?kýsíðÕ?g™P
?ïG7âk-?–ñóÎõ"û?SiÁ9ÙUZ?a¶'ë…Õ?•âg«•ü?•Ú#Ïw?ˆ¸F?pbÄw3G?ué4BZ?j¢98Ťw?¬	à•ób?Ž…Â_¦ñ?ìÐeÕð§?¥ô,ƒ?Ù>ã]áh?LR*´"÷?·A©tV?¦«‹IA^4FGL J0937.6-3358?éÌssó T@+&&ö¶À:Ä"À<6U¸™9"@®É"¾@tþ½	á*?Ãë"ÈÒc?–9;F8YÊ?Ò}y]9!?ýyðql©Ì?ïþ‹ Z›¿çš€'¿í.jÁ¿Ój¿ëíAÄÆn?°äÏÍÞѿɶnçi[8UNASNone?ëìCWF+?»Ù§½µ?{H&͖?~5å4us?¾écösaÉ?ºhø–Ю?ëXΜƒm¢?ÃrãøÌö?…!1¹.†?›ýË9Œ‹?ÁK³zÖ¶'?ÂaŒãM?ëb(Š;?¢Änf驪?•ê]Hq?†"@ér 
?¿­\$jä?¡iJA\\?îàó"ì?˜3_Yä7?jÃúîðÑÍ?gÃßK¨["?­‹¢AÞÄ7?—}&»$êà4FGL J0938.8+5155?Ã^zÊ  	@G>L/ƒ{JÀ;Wѹ›—¡À<ãÕçþ{@Å$ʏ°¸?ÿÚáb†?ʨ3PD¼?²z5?ÙJ?éwÇ·º@ã,€±¿å
f H	"¿ä©£1ÈÏè¿å˃á÷Vc¿Ý÷µƒ¯øV¿ÎíŠG?¿ïÿ÷Ò4ÛUNASNone?G­Œì?'¨cΐ?LÖhVD?E^v¶ò×b?‡Ù`®c/?ü u|u?ï|äRˆ>B?‹N9‹˜.`?AzSù#r?O+7óÓ?¯Jø°ÝP?Š–ùÄ¥å?î,
·ñ'î?\ÉÍ6ûÉ?pþ«IC¢?[0+|	??«Å¸?¯'G¸&œ?ïC´kÆ:D?~:â9ûË?X­/´Ù«1?Olƒ‰I"•?•þŸ‹ëÆ?~J˜zøó4FGL J0940.3-7610¿ïå­ó‡qÀ1sàGÓÔÀ9Ã(xÅ
¼À<'šÈÙ"@}ðpÀÝ@:a'ÑÖø?½=߉'æL?Øü
Ý©"ã@xØ앿ð@Kœâþ?¡Ë¸$Ê׿ÃÈ{ÄÇoÁ¿Ý1{"54¿æZ—ZúøY¿ïÿëJw¿Ø\:~6UNASNone3FGL J0940.6-7609?³4#ò{?ª†@˜?ëšFÿ‰?¶[íë?°,"ßÅ,ˆ?©Áª´§?ÇkB\ÁÜ?ûé	åò?æ{Þ;B'a?ÇOÓ¡)?½J‰li[;?µ;WU¨È?­líVdòP?™²'.ÀÕU?êRøº…Õ?§¥iý¨?¾±ÃƒÙX5?¡hêI®Z?Óv´µ<^?©[Ä)EÉ?×Z{AsWò?°Ã]våÍ?Õ.Ð	P'±?ª_ú£N4FGL J0942.5+7620¿ï\=bX‡"@Aî‰v5çCÀ;ƒS¾ÃõŽÀ=MŽ(LO@ N
/-êõ?û]þ¸Ø#?Õ$¾!ŽE?ÝN']Šõ'@v?<Uñ¤@Ý]Ü)6/¿ïöK¶··'?ï÷
XH–r¿á³"6‹­H¿Î(ú »¿î™ð×n¿µË4*©øUNASNone?îðT¸ŒJ? "åß?'AgE²e?wKÙ Ö?˜ôµK¤?g‰Ì?^®á?¢³'r†¿ì?}ÂÿŠy?ˆQºÍ-ÈÊ?¢ñ¾â š?ú|<5?ë–êOÑ?£ÂÏ0¦Ò?¥
2-Ɵ"?"6抮£Ü?¸Ã–Þ ¡²?:b·"Á³?íïÖD'¸ˆ?"W=».?–ï–j¹Ë"?ˆœ+'$u£?¥ŠÐ'w'¸?mRŸ)ô4FGL J0943.6+4207¿ï'ÌFÑ0ñ@H"­}|,¡À;"‰"hØ1À<"5¬En@¿KŠíÚ9@H…ªÏL?Ñë¹÷Ýò?¿Y'A'+'?ï|ˆçš®m@—¨q£±K?ïË'`—¿èŒµ( 2¿åš'bEov¿ç,	þÜix¿ïÿÿ)@k*?ï™HÁ9ñ"UNASNone?ïê"M±¼?eìÈ&4`o?<'Ùe]#?@ûsyNÎ\?aڐsÓq?dR&½?îǯߍ3}?¬@+¿Bõ?ibI*Õ?|¾ØO\R?¡óA5?ªË"9ì<£?î…ûxº?·¥FüF?t3'èéy?f×yz4Ï?¥æ
¢w5?Œ‰ê²l?ïÇrã\ø?w:å?Aø?S7ÐB"55?GBäèä@B?Š')>ä{;?v<¶ÿ˜j4FGL J0944.6+5729?îÉ75:8O@F¹‰ßrïÀ;Õ09ƒ¯MÀ='¹@ ۑ×-xß?ÿœPbîâ¡?Ñè[ôrƒ?'ÅiV/âq?¶¥ŒÁïÏ?ý§gıË?çD ¾{ü%¿ãøÃ*Œ›"¿åϙ/çNX¿Þ§¨ìMñ¿à¡¿}ƒäQ¿Þ73ÞSÝÎUNASNone?ï¹Ãy"ۑ?{†}~'Ý?BàéP?>½ÓZø³Z?€a&÷6Å?zV'6úî?î¸$KŒÆ? ïaG}ç?f¢«—Ÿ}ô?sìg¨Î?£•1Í;Ã?Ÿ¬ÀÙÀMÑ?íø£x–ø}?'a¢¨g?tÌ—Æ?cxȏ¸€?­ôîó¯¥1?'íèÕè?íÃ/hOðd?›#[öHSË?|·Ÿ.?r¼ÑCî?°%ûâ‰î?›Ã»9½Ýà4FGL J0944.7-5124?ë¾÷!F?övaÍ
àÀ:xÙÔLgÀ<»få@ Ú¤.™p?ý{ÛB±U?ћ)Q2!»?ÏîƒUà\L@S_2•?ý%'6¥®{¿âšÆÀCQŽ?ïÅ2¤—ú]?Òë@Ö3ÿ¿ØîŒÛE5"¿âù́'²Ì¿à¹ë^2eXUNASNone?Ù~7kÞ«¦?ÂÍãɨm!?Ž\¡nãô?‡0 ïOÛõ?âÇqÄX¦?ÂØ_•8@?Ö³äBÅÇ?ËNàTe³?'[¾:°9T?¤è²x?ämÈ	R?ËYž±4U?äM–Ø.֓?¯^H•©&?©vËè²¾»?'ŽhXöËÅ?Ô5øҋû?¬[hÅg¿?æhv»ù4(?¬nó"¦Õ? Gnã@0¨?ªß~xÀ?Ñ&$«¥'œ?¬rÿÿ"ˆŠ4FGL J0947.0-3548¿ß××C›ý@+ˆ7q†UÀ9øúÒ¶À<óähÊÅ@FjpŒ/#@\0LÎå¬?Å=ê†Ç?áÇV +à@ìxc¾ì9@œI1wF^?ï«<ú\R¿à±%q©ˆ¿éñ&³ÈïÈ¿ïÿÿ" 5•?ïʧ߭z¿¦:ÌbLXýUNASNone?êÜìoG%?ÀÉ]؀h?¿ðwݪ½R?¾šh1½‡?¢PIP9"?¢S-Ë©	?èyÊjEÏ?ÍJ}ôë¾n?¶|ð6ú»Ÿ?Äz.³?ÂÚ^<5Šö?Ê»¶x9b?áãBE9ø?²^Ôgµ–?ÍÆøŽ?®æAPn?ʬ–u\‹?©ú|3¸:¢?ìM¶¥?´Ÿ˜õì"
?DÑ$Ýô6?šû¨"ìØ?»'JÜZÍÍ?²²"uø4FGL J0947.8-4234?í¨ÓsZ@ þØôù;ÁÀ:[=~HÀ;ý57ð1V@¶ P¢@°cûRV?ËOÿÇ é?Åëq¾cÒ?úÂ(]í@Σ'•¿Û¡ßyw»¿Ã³œd¥-¿å]&¡ª_:¿äÞ?:þ¿éð9¹_2¿ïÿØ}ZÙUNASNone?à|K¥&&þ?ÁšA'ú'? àã{•?˜Ñ*YÐ?ÜëPAD?d?Á…ЍY˜?鞄Y¡
D?Âô~''Gç?yv*²?†@k"¢n­?ȽmåËɝ?—žE•å?æ®ó.T?­Âµ€†9?¥<z30‰s?JR	"ÓŽ?ÏõC/$S?ª³Èõ8S^?ìP©L¯õÍ?"™ÂÏÈ=?Ž`Ò#³Ÿ?sz;œD?¹®›V	ݲ?'¿ýl64FGL J0948.0-3859¿ÓüŒ-râ@&y*Qã!£À:¶¾(Å(À<£hOt²@›"j8-@A³ÿvmE?ג¥^žÆÕ?êÅÂíOú@'ë¾íç?þ õ;5?ç÷X[á¨&¿ÝñÆ@ì"M¿ìþ£^"_ô¿ïÿ'ãñ?ïø¼ßï¿@¿ïûÂ-·sUNASNone?èyKœÆ…?Ã)+{Ú³?º!gœ6œ?·þÉbu?ÁÀÙªš?»–°û[îð?ãûûò¶?Ðé@;4M?¼éÛ9iá?ĔLÎÆ(`?Ð͑M'¸?˒gۉ'Ï?ãʟ?ŸYÊ?­1ÑõgAç?ÁÆɤàÊv?¤züÒe˜?Ϲ\¡Îd?¦È«¾´.?æ"è¯a«?ÁøþGÊ÷â?Ÿ/QƒW'?§¾ph[?ÑÉK¬Ù3?Á€½oÙ4FGL J0949.8+7551¿î61yc‡ÿ@B?ÖbwÄ]À:îJÔ9¨˜À<ÚµŠè@ø™Iè^?ÿj~…A?έ©MÙ?Ó¦¿òɶ˜@¡/à˜[¬@‹¸Þ6¿ë¸Á>#Q¿ÉÿÓµI¿àÃ.ô	Q¸¿ä ¶© ¿èae`,¨¿ïÿõƒ¥;ŽUNASNone3FGL J0950.4+7550?îþ'¢z?"ÔVë÷ùò?€$¨(»ÿ?{È·k¢¢ ?˜·7¨²Ø?'oݟcw?îDhŸO7#?¢ž0͛0-?~Âh¶uÃ?…òµ:ã?§á)	¿%?Ÿ¸¯t	Ä?ëÙã¼È?¡oáiÆÞ?¥ÔƏüŒ?'ýs%ð+ú?¶F~Ò6±"?——ؘŸV?í»š—¥?'œû>•,?"3ë]Œ«~?|xJs­á5?ª¬`ÖèX`?Þ"úªÓâ4FGL J0951.8-3711¿éØ?ì¡uÓ@*-À3aVÀ:µž·æ‹»À<:îí‰@AÜ¢òô@¯BÇ$í?Ö9íAat9?î~;¹ÿk@>l`{jÚ@3ô–#î¿ìÏj¡^‰ù?¢Âæo
Nã¿ìà=lòò¿çí?3¶?¿ïüBK?ïęAÚëÉUNASNone2FGL J0952.7-3717?å^Vfyœ/?É0'`:¯*?Ãÿ¹Ü×?À‡Ó™±¿?Ƈ¬û²o?^[Ò?à[—GIª?ÏAïoMf?ԆL)Yc?͈H¢?ŅŠJˆÚ'?Àzä}êçU?äKf‰(¿?±þzkTûÆ?ÇÑAâ'?¬µúŒÑ˜Â?Ǻñ#øÊå?¦€™ÑF?áS'ºøi ?½'j1t¾?ÐRî«a^\?»HËñÂ?Ê
ƒ½[œÌ?±Ë˜in4FGL J0953.6-1509?ê×I"¼K(@=šO—íÇïÀ9Î,UÉ`1À<ˆ¢Ù´;Ü@"²U}5
?ú»	 :2+?ºžolIP?å(U{\˜@%%"1zÌ@9RIMü¸¿í<Lû[V?æžÞ&'d¿ÉMgfìs¿æ	s˜Ôx¿î"žã…uö¿ïûÌßÂðUNASNone3FGL J0953.7-1510?™É5!ß½4?˜Û¾Aj¨Ì?î·°H'ì?£&·_bÀ?Žƒ¶'?"Ž¿¢.U?–!&6¥V>?§©V3Øz¤?î@Å=– ?³Ð[Æjá? ãƒêß?£úðÁÖ?¢êÂóüß?'¢Ã)˜X%?ìf^ĉ?Ÿû!°ù?³U³á-B?•ÿu¢æÅ0?"kŽ²¹)ß?'©'$€ùÿ?íÁr•6<?›fýáAϐ?ª3UH?•jøÿÓ4FGL J0955.8-4106?ép ¾*al@%ì|•|ÔÀ:@\78{rÀ;¼$·om@ÙÜ»W@z[ñ?ÑsÓÜí?â*8ÅC@Þ¦c¬wÃ@]!)ÆM¿Õ§ÕÜëÓοàøi"®U¾¿êû/—@ú¿ïÿò(¦è7?Ѩ©ï?çjNRsjUNASNone?ëK§ÛQæ?¿ƒÞÕà›?±"™âªOä?²_W'Úž?´'BÌ°é?·G¦1vg?éùªYÍ?È<EL…é"?¬ÈÂë:Ëm?ºõ5?®¨<?Àéh›Ìáð?Âlx-_‹?ã(«6%é?°0"ìÂYö?À›"eëã?¤7Ø,?Ñ`ç`ï<?©•â,^?ë¸_(¿‡?²u/ç0'Ä?€DPooÛ?ƒQ®‹3÷?ÀC7üºå?±â‹ÁkðÉ4FGL J0957.3-3851?ëóÏ^ç0@(ú˧2ßPÀ:sö•3À;í┵.K@¬Þ½e&@—s\.Ë?Ñ+^×{Ò?Ó
©`áí?ü%F
¦L?ö—‰çtî¿¿ÞqOÎtm¿ä[Ò>%Õ}¿í»ñ³6"Ò¿â'¢;(Êú¿î»Oag#%¿ïÞú̺XVUNASNone?汉‰ëþ?Æ4!ù}Ò?ÃçÄ0δ?Á¬"¥ˆY?ÁR§S¤?½0Öç3y?ãž.àœ?ʨÍxyÿj?Æ&Ö|Ly?ÄI"ø?Ëa
=A‰?ÂÔØ'Ƥ?ã+=ãºÄ^?°3ùž+7?Á+%§ Lò?£ö/CÌ,}?ÑñdºPË?©ÿ#Ñ!HÔ?áI|1?²êÑ1Sèµ?ÈeNlÀ^G?°¶%gXï?ѪƧn¥?°BVc¢»4FGL J0957.6-3051?ì6ÞãÈd@2µ,'¦77À;(Òü'¶vÀ<šˆÉg½~@nןc³@9lÅûø4?ցùje?ì)KRä©b@
´¡\Üyé@re"C¡À¿æR:Ê×)G¿Ö™}j¿æt5ýö¿ïû©žõN ?éŸ@¤Šä?çÂ)óUNASNone?êŒ"'¦s?¿FSOƒ ?¼DÈ_ˆ?¹p  ?¯MNvˆÛ?®@	H'î'?éôÙԂ?ÈËw'ÚS?·»'#<¿,?ÃÛ$µ†øÖ?¸¤20=?¶I•'=?ä¡oL[?°6ïé^?ÆdøÖá?ªw@œ Q=?ÇKö}÷³?¤d\:'›¯?í"r~™ü?¬f>ù ?‹çû'GpÔ?–«t7Ôû?°_l˜î*
?¨':$vN4FGL J0957.6-5208?²ÑÇQp‡"@ɤ^ïÀ:€<_+߂À;Ï _Š@è°XÍÌ|@X¢t3¯?Êm§"n>ø?±´p	¨Ja?æͳaÁ»ø@Xœsé†Â¿î;Ɵâ?ïöÌD琝¿áãñâ0a¿é+ñUBQ´¿å"†ŸìÄå¿à—|ÞÍÖ7UNASNone?ì…–"9?²¬,u— ë?há‰'¿=f?f	ñþÑ2?¾¼Ëª
äF?²ñß¡V?éVò›TT?Å>
KÞU?qäåGâb^?"ð˜Ã$?Êhp¿š?ĽAnP'ð?é.üDƒ?©ö˜¤³<?'ük.@S³?~h"p?Â?Èè&©'Ӏ?¨I¡sƒ¨?ìÛôO¦Se?–RÚaÖÎ?r	NȇwZ?cJ(X$G?·ÿȖDí[?–c*öå(4FGL J0957.7-3510¿ïá_ŧ-@.Οð˯–À:svð!fÀ<(˯–[!@Rqé&t´@!Mryš ?×Ëq'úä?áƧ"=çÂ@	o!öÊÍ?ÿÅäÆh¯—?ïú²]à°Ú¿æˆ(Øîn¿êædþ²M¿ï†Ä);
?æûÎRÞÊ¿¹ŒÔ_":UNASNone?îî'N?³rg¥•Á?˜,² ø?ª]/228ß?"'Ú,B
?¤=ã'~ZÏ?ægŠ))?Î7eGXÍ
?¿¬ZõcB?ƌA-\W«?ƍ¤OQ)º?ÃE‡_êAñ?ænjÅåX?ª™˜ÆÔ?ºØ–¹(
T?¡s"€
=€?ÈÛVøTew?£€AXEc?è̉Šd#?¼M‰Ðxµæ?¢Žº»ÆÃ?©% xx?È-wë'}Å?¹ÆCó¼Á 4FGL J0958.6-0522?æ, s—@=@BŒ>§¼À;"žõ#-,À<›w3=D.@ØZ°O¾"@²¾‰¬½?Â9q{BkŠ¿±"Žg·IX?í1išÐ?ù͙Ëî€|?Åû`ž{U·¿â;}^ûc
¿ìúþ£ßm¹?ÙÈuO7u¸¿â¥ýzïð8w?Ò~UNASNone?ïΊZ+?—±¯>âœ?|‹#qx?Š»v6Bg?"âÙEØv¿?'clgûV?ïPé‰\±?•>é+‹U?aór‡s×?z±ž0®=?"¤`ƒŽnð?'´+8n¨Á?í"ìè¬?˜õÀ¨û?ñ,k
¢?t
H"¾`?±àUؖÉô?–Íó¿Œ ?í¬A¦É? Ëå*©+ß?•YBPó¢w?"ñÐW?ª'ÚÆ[ÂA?™ÔÞ@Y¨/4FGL J0959.1-6441¿ïâœU>S€ÀâDÀú0³À:˜8±ø50À<§÷*ni@Á¥"Ò@-IÿþR?Ðô«£‡Y%?Î"øþYà?ý·}°/@¹‡!m¿Ývz"ð¿ç—ØÏ9Ž—¿çW\¨w'î¿ÞГásÍØ¿ïÿýF\I¿ïƒY¡\ºUNASNone?åÑK]Ãé7?Á'´{Þ÷?'®—»a?Š&ÕpÖ|î?ÓENZü|Þ?ÁNý…&?߾ŸF;?Èëî`ñ›U?y°5M\–?ˆãeT¥b?àCÀhEÂ*?ȸܲã×;?çÖ.æk8?¨Ær»V÷ä?¨«$_ú»–?'E–á?Ê|â,g¤7?¤vú*ÙD­?êMˆ¯V?£ÙÄS¾?Œ·ìÙ5©P?xÖ!¿<ç?Å;¯M?£FÚ²ƒ4FGL J0959.1+5719?ÕßÆcú@G¥"À%À;b,µj°À<"φ»p"@‡Ž6¼@ÂzÞÃo?Ã)2(q8R¿¶ï.vŠ÷?ô`­¤éXõ@6á¿Î¼?ÁqËýTª¿êB±(+˜¿çc˜UÌ»¿ëõÖEòR˜?ØÓ P—ó¿ïþ±¶ÆÑ
UNASNone?ï
,˜ä¹B?¡ÆñIÆt?}õ|oM¬?z‰:ª"?–Ý
Ç¡ÄR?+:[óqþ?ãr†j?§þ£JÏX?tawêÖ@þ?ÚÐ.ß?¢‡òË|Ñ<?¢˜ÑpÒ?í¨ZÐ{˜X?'v™]l½Ë?†œzh'¼Š?yzƒ‡ë2?¯Ó4^!Ë\?:â3¶+?îÓJYø"B?"n8mY¨?UF4§Im1?\{AAa¼·?¢!(»<p‹?"!+ÂB(4FGL J1001.3-2040?ſtP{1h@:ê7&úÆÀ;LÇ+£ùÀ<½oe©P@ ŠUŽ¡™?õL«	-¦+?áÀá?µ"?ã…ߨq£±@tœŠâ?ôÜþ(º¿ëì&ďç?ÐݧESÇ'?ïÅTӖëi¿¸ÜÐ{)Ñ¿æ—IÈ î"¿ïÿÿ" 5•UNASNone?ïÇOÞu¨\?V¥ˆ.åË?a.֟îB?dRUü¤d.?sÁÙÛÚÉ?}v«ë ÑÌ?íV9A"\?·©Ü.Xä¶?œú‰Eñ	?­Y²éŠýT?°~«äw˜Þ?­RF—Ú?ìemñ*Øÿ?¡£üæ €E?–öh1.qî?‡ R,Ï·?·öj]›‹?žÜ¥ˆ¼>ä?êã퐦£O?¯V¢ú>m?"
ø²t6?•#ƒá@Âÿ?Â	^O$;?®™9€íQ×4FGL J1002.3-2810?ëŸ\¼!7@5k»ƒÏ,ùÀ:әt°¬À<<íÜçÍ@n݃S\@!]³9}Ð?çÓÌ@
>?íU/<-­¸@¦ó|cþ­?ó-ƒ«ñŠò?ïö%÷
ø¿ß¸ç¨eÝ¿ìuL}‡\¿áó{jª¿ï÷dP±¿ïüK_ÏÉVUNASNone3FGL J1002.0-2837?ìB¥ôé79?ÄmO›'2?»¿@Ã(sC?Ä`YªB.Ä?\|¬n—Ã?ˆ—Jx
?Åûï"~?͓–dn4À?çk~i^êÐ?Ò>4ìS|Õ?¹¤Öÿ'‡?»YQ(àòñ?æû{
­`?¬/É`3?½þë\%H? EZÎí?ȈÃ'7Ü?¥…š‰n¡?š#4|òª?ŸRO©˜B?ë¯äŽð?ɪ.â•?À³°Ï€ì?Ư',4FGL J1003.7+7049?½½úü#ì2@D4cŠ	À;Ä5LèæßÀ<ÝrÐ×ôH@ ñc='Ó@
&ˆó?ÄÐR¾=èÄ¿·é¥´¦?퉎;Tj@³sŠfK¿åV'""F¿ç5:	Iú¿çú+	™ö¿êø¥˜«]?ÊÃgÉ<õT¿à•½ÀƒUNASNone?íÖÍu¦@Z?½]"`)"?j/Ÿfÿ8	?}7ƒšçUÑ?°xW–o?¼t0Üh,?î¾×4¯9o?¥hF¶¤8?k!Éx'?€×q–±?¢`pŠá?£…CnWÖ?íšùÐ`ŠZ?"^"­uÁÐ?z¨ì5ƨÌ?lî©w?±}¢¹ŸB¦?']WÇItÈ?î!Œ#Fdº? ´'_Тé?UVj{(»?Züû1÷³7?­:»EÛ!? ¼Ê¤¸Ä/4FGL J1004.6-5215¿èê)T@5+Z÷[À;"÷8±!vÀ<‰E=÷²T@î­94?ÿ÷i=±;w?×RaA
'c?éÚÝfx@¥ߙX@|´>
§¤¿ä9Œ~($?ïøٛhÞ¿Ô¹+ºîÓÞ¿Ýq׳°œ¿ïÖèå1G¡¿ïWîÕSUNASNone3FGL J1003.7-5215?؆1
øiš?Âô"µöã?ÈØ»8×~V?¾	iߍŠÖ?Û
qU›×;?ÅàÙ	P>$?ÉB‹«:e?Řv8?Ð͉mÚr?È®¥8è?áH˜^¡ùd?ˉºn»??ä»ʞ?°}®ºÿ`?ÁJ‹õ#»o?¤œ
3‹!?ËÉpàd,?¨÷mh*ã?Ýc|l!O$?´	}ÔvSL?Òã­""Ä?µªä=i´?Ïq¬þ—3?°òŒAu4FGL J1004.8-5250¿î?Ä!hÂ@—a_–iÀ;9
ÏÌ[ŽÀ<X·Q:…@$Þ.ŒÛE6?ø†Ì7{—P?Ňϗ­[B¿·¸ËŸ6wÇ?ù¡cýÖZ@JÒ1e©¿ïÿ˜f"²Ð?ïÿõ^'¿¸œmŒ?¿éf è¿äj&¯—1à?Ê[å™w_ÞUNASNone?átÖôØç?ÍrIU«ä?_ Þ'9ç?f¡sÉxOm?Ü÷19ÙËù?Ísii'g©?Èˋ!m?Ç	,*_m?™¦0;‹?Ìæ*I-l?éV¶žãÏ?Ç?~áC?獪_ô?«/–ó%±E?''µ.êêû?~ìŒÏ›Óœ?ж¹Wð'h?ª'¥˜óm²?ÎS&7@n×?¾èÜyÊUa?'üºòxfŽ?llíã?çÛPšœ!?ÀÊߤâÃC4FGL J1005.5-5708c?äTÂÅÀq¨¿ór˜Ù€9vÀ8ùáy,;ÈÀ:s™LlÀ@<½J£½@7­eÿ8Z?Ê»˜Ý\#?ã·¦±.@ö£ð4±@ðbF¿íÖ®b~zY?é0ðÎ3Õ¿çñûûŽ8¿ìài·ª¿ïþ݋`ñ²¿ãÙ}'ÕUNASNone,?¼·×2å?´ëvŽkø?е2F¼?ÆÁ	êfƒ§?äfD‹ú[ ?ɟ{•Ææf?¤ðòØTZj?¤ÿws¾K?׏"{«‰?ÉóÓUHCG?âé.Î<ä–?ÉRó0G?ÁNY\Å?¢ì½›ÿS?д`lªÞ?¯hp£Då?ã`v¼3S`?²è^EÎ?‰ÖY	ß?qzò	%>?Ø^Ô?±Ò?´ŒÖ²Tj?ã"I<{ÿš?´f)@¹4FGL J1006.9-2806?îѯ¨#Ë@6!>‰¨‹À;=Õ¾
iÀ<m7Žâ†r@ÅñÞ&Ò@™þ†ƒ<`?Ì™<§{/?'ÑŠægAq?̃ÛÂ3@‹µ`£¯?ïåe¶™…?ì†e	o‹¿ì£é~´;¿Ø%}}":7¿Üøe-×)¿ïþ´ -UNASNone?ï]DÉ…?ŒÂköôƒé?mZs,?j­Ï†«Ê?¶ØwìN?Š#Ó%ëe
?ïI½É&A?˜(:ÁóÌj?Z<ÝÁvÞ?v"sTJ&â?•$xÿ {
?–%®¬ü'À?í#~ãœ?š³Y!?†÷B?3óÅ?y­`sê'~?´ ŸL ø?˜D6-0?íÿÂÌØÈ?•l™óå˜Å?ˆÞcÖy?}Øû[¨–Í?©ãì:<Õ??'ǪÀ$¤4FGL J1007.8-4514?ΞÅÄVô@!>—Ðk½¾À;^(Àª'À<p‹â÷±}@!ö¤Q-š?þù²©5?ÆÛK•ª¡ª¿²ˆœFG7!?óõ«é'v@vä;ÿ4©¿Ó¬ž"Í¿áw™:¿ê®ßa$F¿ïÏüE±?îüwµCCL¿ÒP|VUNASNone?éh¯ï˜?Áp<…R"Õ?T*¸t=?QðÁAˆè?Ê4ïùbж?Ác¦»	Ñ?ړb‰{Äa?Îû<uZ1?‰«7eê\V? €m6:=ó?âO¡Ýªt^?ÎG»1"?èЗÙRAX?¦¢9¥>?Œè;?zƒT0'?Êï²ÃJŽ?¥Ó$Å&n¹?ël`Õ¿0a?µ]èj±ï?Dj¯XÐ5j?V7'ï¸U?Â:ùªnH?µ]Xa"¯ 4FGL J1008.2-1000?åzñ+¤Ò@AߥÁƍÀ:7äÞ;ŠÀ<PP¿54•@ãá5E@)ªIë?Ãb'Z/÷??µvÄ­n§?ëýdQµ@gõ†Tmk¿Ø³D›:ƒŠ¿èfœK›à¿í|KÀrÌP¿åï`«;'¿ï÷¶O²Å»¿îʇB'UNASNone?ïŸÙä>c?'úç"g§=?~·Aýð	?}±œ†~?q[ËâÞrÅ?q`9ؕ·×?s‹ôH?¥çýÈ?|ì•lÄ?u5ç^Åõ? "»4"#?Ÿ–ÒÒyÍ~?쟩+‡ç?;"@ÀÄv?˜ä:gŒ"˜?Š
rå4?´É©À›ã?—"4gž$M?ïµ+s{~?ˆÜsAc<?'ǼØ€ã?"¯uÞ|¤ª?‡ƒ;çp´?t…»"¹f4FGL J1009.5-0034¿ï.­+`›@Eß;dZÀ; ¯7'À<ˆ©í¤³©@Þ@ÌùÃP@RpEy‹?ÔÅ$'n|?Ô­ÎÚÄU?û¦y–ÄÓ@
›Ž¹¿ïÿŸ‡ð#ê?ïõ}€3l¿Ý ó*.§³¿ç¦Æþ¬˜Ð¿ãmZ@¾61¿íÚï9ßßUNASNone?í<zMYžã?¬Ž6Ï?"§'bÌÛN?{Q¶ÊÅì?³‡;hÙm?ªñ/ä)N|?î°ý;Á–?¦îSšQ÷?_/"쮑?‡Ó"žÏû¹?«$G»?£ÉŽÀv4½?êô^¾[Km?¤Ñ"û>ØÔ?¨H½Ýu?"#ðÇïGs?¼8«kb?ŸÃÅLecå?ë߃®¨ž?zªua?–ëݺ®ÿ!?‡͔Aiµ?»Hð‹ÞûL?š®,x±º4FGL J1010.0+1416¿ìPÚÁŠ¬õ@I*û~ÿ—À:ëG‰+MÀ<eÝãu…¾@¬¸§{Úl@L®ì?Á¸#G'Ëw¿»wۃÉΖ?ø†!Ðý?ö…ÓÉÁ)«?éÛÁÝ/›¿èî÷ßËF¿íŽÌKD¿Ç³A¶X¿Ñ(}ãǐ¿ïÿ^º z^UNASNone?ï1¨ÔÎ??Ÿ¿ÒíÅ"ý?ŒDH#m¥'?Ë'á_Y£?‡Q´ç^Ê°?˜ºÒª?í÷á‡Àd–?±™òXn¥?‹¶°u
?¦/júúÇÒ?©";'4f?¦ސøÃç?íǓ	9²?šö¼$•'©?''긪ÄU?‰¹P9´ ‰?³•¹‹Z?—P¢ò@ªz?íg«¹?£ÈÚ¯??"gÀ'Té8?"ë™òˆr?¯Ó¼%Î? ‰Š¯L4FGL J1011.4-5729c?ïýÁìôàg¿ð¡ÒM?MôÀ8ÁÚWÏÊ®À:Fá$r¦@kŸ~Šõg@b¡ Ï?͹§@¡/æ?ÖK2»"@÷ñsuB¢@|{ðȀ?ÛªcÇOµ?ÈTZŠ»x¿ç½¾a¥"¿é¿*þ~ð¿ïò-DéN?îK®UNASNone,?Ó|àÎ }5?Å·[)ËéY?»'kÔ£s9?»¦lí?âÜ¢[Rþ?ÉxpØxï?²öt)`šï?²=~Jë8²?¿Î ÞÍîç?½:±Ä&K?é§m^ú.Å?Á/ÅN×Ç?Áƒ¡ã?¢Fù×v?Åþ]¸ŽÏ?¦†­5{ÿ ?æ€*"´T?¬	¹d@»?ŸW}‰ƒ?‡¹ÄR‡?ÁÉ:nò
?¬)¾ËL?ê"Õ{§1?¬iW1"Tg4FGL J1014.6+6126¿¤ëŽðþmI@Gsý'w>%À<#§ÝÿúøÀ=k-àãÛ@Ãf0‹Ž@'9¾g¯<?Þ:Gĺ¯"?æ"äÁ5>ü@	~?íëÑT›ä¿ïO±^p‡?ï·l]¡E࿺;ùÖEF†¿åèQ'¿è&ch¿ðUNASNone?æÃL•?Ëõáj?Ï.÷œÍµ?Ê<*9>!?§o+Ãw™?´IPLt¤?×pþ€ò?Ñ×x9¬EÛ?߇¨Q¬§õ?Óñ–¥Ç#?Âu_‹®2?¸À
«pgÌ?æŶ`&¤?®"š6C?ÁÙAÈñ¦ƒ?¨TÖ0¨â?Ãä¶sÉ{?¢}çðvP?Ç+%0Ÿµ;?²£Ù…Ø—û?æ"S>ŽN?Á|]sЋ?½‡®4#?·¢§C§Œ4FGL J1015.1-6353¿åP4†'!À.ÝÎ|Ð5À:yªÜ·ü[À<(íA°¤@z¤®Ë"ù?üü|¢èÍ´?ÓTª|?ì?Ü9ïô8@—€)†?ú}YÊ¡¤U¿Ô(ðd+£¿äõiøØÄ¿àä›ök+È¿ß,qãr*À¿ç'vµiù¿ïþÎÝHEUNASNone?Ü·u÷ó?Áõ›ÂK?¡äê"5N?"ƒBC"û?á¯ä?Áì™pÈh?ÌüyaäL<?Á-¯ì0
?"©`µmZ¼?›¦`É9¼?è#–¡Û'?ÁAy¿ûT?âÛÇþÀ•O?°ÇÌö|;ž?¸hí«z?¿]}CfÚ?Ô.O‡öÜ?¬Jh8"l?ÝZŸ:î?®–-£?I[?©ué8…g??•tfˆ(Ƚ?ßv£Áã+?¯-šRÇ=§4FGL J1015.5-6030¿àÈCë^ª¨À	¾±›îÞpÀ8¼o´ëÀ;{'¾Šë@ÁIÿþR@Ž¼g#ü?¹µ¥ÿ-?ÄÂÇû¬´)@¨É¸EV?ö`õ˜ó×S¿ÁO¿Ez³z¿ã'Ž½É¿êw$>£©¾¿ëèU{\˜¿àÑÉ oâ¿è½Êeê?¤UNASNone3FGL J1016.5-6034?Ùz¹c –"?Äœ:¢©Ò?¹lVåŒ?µ°Æ8;+?àq¾0Ö?ÅÕ¾Ÿí'í?ÂðË×¼	
?Ã+o¥>?Áulږ?þ?Â'í2Í{?ææqÓkm¾?ÈY €Üñ‹?Õ,›½}÷6?®•¨äÞ#›?¿Qˆ#ºH?¢Ò‰´?I?á\?®™sùE?Á¥õ'ç_E?¤¹Gà'@?Ï¿ÞCÆ€?µböIœ+§?㦋%¢Ï?µÆ"ÑL`4FGL J1016.1-4247?¥íÆrŽ¿€@&ùþɟãÀ:H¿è+ÎÀ<L 鄓x@ °æãÏGÑ?ûtyŸ(NÔ?ÂNÔ8üËÃ?Ä+S?î¦@—ԝ{¦@&ÎEÃö?æúÂG¸¦¿ê1s	â×Ñ?æ±x7I¿ÛX'}ÆV¿Ö8\½Æ¿å@W©4APUNASNone3FGL J1016.6-4244?ëBÄ;W«?µ1°µÉ;?"ÆÚ
N6^?ŽpÞSx¼q?À|аڇ?³ê¼Aìs?êVŽN˜R?ÃTªÐ˜?}/;/h'?‹¹[öCv?żLì$B£?ÂÑ~{ŒìÝ?ëšö­{Z?¢¢	¿?‹›8)è?{ÓH©m"?¿´é!ø-?¡s¡†ÆÁ?ë0³ø&¼}?£äÖ¡õ%?‡i³6Nl?ásÊ~ûÒ?ÁƔì.?£«ãû#!ë4FGL J1016.2-5729c?ëìõVƒÅG¿åًâvØ$À9[ãU¥NÀ:iÀ¬-@:šœxò@?ޚTª|?È<¨èA€?·6ј–?ò¸ ?¦=@í±GC¿ïø§¡o%þ?ïïNlta¿çU%`â˜ç¿æÓ{rg%©¿æÕ²^·po¿é¯?¨¢UNASNone8?•öÔ-Ò]?·,Ö¥ä?";Ɲ¼ø¼?–+Žã‹Ü?êÀ¤££?¹È£Dˆ?ʂž5'?ãï¸ðv$?™¥Ç‡úۜ?¬²qµ4Uz?è'Mœ [Ù?Ãï'VO6M?ÄgÈçɸÇ?¥~Xæèìä?º+†øÇô?£ŠaÔ^?ç «.xÏ?¬Ðç(¡?ÈmèwdÎ?­=¥hõÝ?›#ÈFŠ´)?ˆ…e¦¾(?égŸòvÛ?®° 4¬ª!4FGL J1017.4+5956?ïáM‡ó)@HQüLYÀ;¥
ÒÁÙÀ=
GR¤è'@¡Y¢<U@´'òÜ+?É -à
?˜K­A[õ?ÐG¯Áú
ó@a+´ä¤?éuv¿ê–ºö6¿Øv'•p?¿èi?Ñ&N¿î)gØVmË?éÒܱF^‰UNASNone?îÁ?FNÎ?§Ú~'‰çÞ?s\,³I¶?qVBWˆ­C?¬Èfˆd©ð?§&îòCwæ?î§b"¿L»?£.Çµ§]?i˜ƒ÷¥ƒ?waÃ~E?£ðOt™ùö?¡ËCÕ¦z"?ì¤'ÚÂù ?œÆ·[÷\A?•€P¶¹ ?ˆ#哘t?µ~½º"–?˜böô×Ù9?îëüsĉm?Œ¨Ín£3?wB"

U°?p£$¥0¹Z?œ¯Ì"ì='?‹ÏÔ®'U4FGL J1018.1-4051¿æ"VÌё@*"4çhZÀ:¢ï	7·&À<;EM*Ë@I'VT'@E®æ1ø¡?˂ºZ•?ÍÔ`)‹i«?ÿñõ*¹çî@ØÌàBö?îH`A]ò¿ätcI{t¿ç‡§ßW"æ¿èa3¡˜¶¿êÐ0Áhë¿ïÿØÝý ÓUNASNone?è0¬‰`?½É¨^ô¬?¨r.¤ƒÈ¦?±0(à>õ?Ǧ±¦hèT?¹¼7æZ¿–?ês嬐y?Â"—Ä­?–*Ý?¥X¿´!h?Ã×k]Â?ÀSÆ °mÆ?ê'Y8Yø,?¤Ýµ"QΈ?§"	ôN3?",yÕ_^?¿Ü1v6?ŸՓ»?é'ÍtÁm?Ø!$ÿw?¤U¡EÕH}?†ßl¬Cô?ÆKcH·¨+?›Õâ N…4FGL J1018.1-2705¿Â…âÚ¢šÂ@8u#Ä*fÜÀ:hõZŠÀ<8a|ÚQ@ɓ¨=÷1@˜ºvˆó?ĪՁ&[4?Á½¿~/°È?ú¡Üär@!͕I¨À?ïý:óñÔÄ¿åvv½Ì¿çmâ0·-¿éŸÚÚ®7¿ä:ˆA'O¿ïúp &'UNASNone?î2¾¥@"?§Kû
'Ã?ŠÍqô[(?‰R³ïRI#?¦ Ã(•€?¥0"¼Àa?íÁê!Rj?§2öbK?‰P<æ@ï?'_½þnÁŸ?­OÔZŸ?¢<c=i›?쮛AŠÏÉ?œI<Ç®tn?'ØêÍ°pÞ?ƒqi
[?µÔë@=e?—à)Õy?ëÅR«ÿ:Þ?•Ci»zêm?ŸÖ°"|–?…~7Vál?¹ß¾œ!	ç?'Y¤sõm4FGL J1018.2+0145¿ã°/²š@F³jçÕfÏÀ;$©Á/À<±²•"@]ï-õ±?þŸô╋î?ٔ"â-1<?ïýwå?@dÞÁÁÖÐ?úØ]å
‹Y?ëÿDïY­¿ç˜>»&²¿Ê7Üæ"¿ê'äÏ"£¿ïý!(n´?ïòH¢0AUNASNone?귃ŸãÈs?º$ÖyxŠ?¤Ôñ×±?£4ãS5‡?À ¼CûM?¶œhÞ²?Û÷å¨×ù?ÓcnË
uì?ÙòDCñQœ?ÔÌ짤™Y?Ä+­fˬØ?¾Y\¤Xwo?ç Ì"×°?¬H}؝e?ºQ$Y?Ÿ¢Åâ*`û?ÆÖ{%Zt±?¦'ޜÁ?ʈŠxôP?²¾Vš)ý?Öìàð–t?À¶)©8&§?ÛÏ¢â•A†?½€»õ¸4FGL J1018.3-0703?ÑføÌHÝ@CÌÅûø3ƒÀ:¥·gà¹êÀ<c@ìF@@\ mf@"V^±f??Ðyu'
5ô?ǟxÖ«rà?÷‰÷/væ@­9ó–»?炙›L!A¿å)
`EË¿ß
œ¦"Sß¿ïÌdAÈø,?ãèߢ'fŸ¿ïýŒó˜épUNASNone?îÃî|'?£7Z‹–¨'?qCˆ¼FV?uI}gW?¡›T´Ë-?¡èl"ò"ƒ?ïüR™D?¢ÌRbfNm?p~irŸ:?Ëñ)'I?›Ûg³/²?šÿ§Ý'W?ì^Y¾¡¤¹?%€ÜUZ?•OhL•ƒs?‡ôóõÐ[¯?·¹W÷ÍyT?˜%UŠµ¡d?ï})¶‰?ƒÿ'TŠoþ?AúÅ^?H
Ɋx‡?™a¡ðþ?ƒ©Ædö"²4FGL J1018.4+2210?ÜRi?@Kƒ9Ÿ]þ¹À<jQÎ_À=[Ëñr@%+¶ü?ñ¥"}c?çd#Ë·#?ã,ù'þtæ?õáÄüó0?þD!!㪊¿îëç?ï2Ôy±¿îéDg8~¿ïš|¨"2?ïÙ|s%'?À"v>öŠáUNASNone?íñ‰Ì€Ú–?´'±˜'²Þ?xÛÆp@?"<Á¢ ?­Ëêiï.«?³»o¬W Û?ë‹èeû?œý9¾í:?£S#
·Ñ?¸w _s?¹ýß<7tD?À]_žX@Ö?êk'Àî?Ó?¨ âKèl?¤9'ZOKª?',>¸þ¥ž?ÁEe³-Ç?¦0°ç"â»?â±SŸX–j?ʉ^	‡æ³?raAºH?ó™s[+s?ÚUK<õÌB?ÊÅ`p^fñ4FGL J1019.3+5625¿Ü"HocÛ@I
¿cíÀ<©.bÀ=5óþj@!
"´ÛŒ?÷ÚWdjã¤?ÝEÈa-A'?àt†_U% @)!ÌÙb@ÊO*Š˜¿àÜäÝdʅ¿ïýE¥ü~k?ï¸7îƒ×¿ÑÏÜâ¹_¿âA¿Þ&çJ¿ï·a–5UNASNone?îþÙøÊ{Ä?š¼!j9{?náZ
dù˜?nPÁ''X"?œH•¥cè\?™_¸àp?îÃ[&(–?¤Êš'Öã?k"fŸ#3Î?€ŒbÃ'5?¢3Ãl?¢– @œœ<?ì·ÑìÆJX?¢epR¥Á?‰3åͧŽš?¥š¨Ìo?·óà»d?¡¾6zõø?îû5ëŒ?Ž÷6ØI?VÕñM2˜d?Tn­ÉÊÏÄ?£
Ý«3?Žxد±*4FGL J1020.4-5314?Ζb¿@	•,ß?–À:Ž¸c­OÀ<Jr&Ü
@âhgs@½ºŠ&_?Îÿ*˜>?â_t¤íŠ²@)M<É´ê?þhà;"€«¿ïÿÞý¦ßR?ïÿÞý¦ßR¿Ú)ÜÈBy¿éˆÛÜ4I¿én"‡êD­¿ïóóí£*UNASNone?¹Š?r¯d/?´*ÀXVH?é: †Å¶w?ÂwêÔ8?¼¤¼W"è?·Í`À·?£èº|vŒ?¦ŽΐXã?á b'48…?̯³hú?ÛB#Œà$?ÊÌÔ1f&œ?ÒÒá©5?¯§û¡k?Úujƒ}?µM¿> rn?Ò·³Ós²d?¬,;œ B?±ŠÇ¨Ô?"þÛ -,?é"ÃlÅ:ø?·q²¬¹ï?¯æéf¿µ?µ¸ójÞj4FGL J1021.8-6308¿ßW`0À}VlôÀ;+Ò/]À<'Ÿu{­ @!P-"áô§@¢>ü•u?Ä7A"Z¿³bÎ~€?óÔ*tGÐy?÷Ûb¯L´9?éJZÌÕ0I¿åÈÂ&*·¿è|"Ý¿äå¶rî4&¿ãžÅý0B? ý#à7–UNASNone?Ý9ö\ºÊ9?ÃôÊ!J`?lÑâ;ª?c—˜Ñ?áF2ïg'Ç?ÃøÚóO«?ÏîÁ"Að?ä7ß©œG?'C$oD³!?Ï•ö'?ç»C
>·?ÆIÓãU5?ç÷€­ða?§-'#i*Ó?'PÀ¢‹«!?v!'~L_?Íù}èöÉ?¦
çü"d¯?Ò®¤Š3Ñ/?´úà.ÕñQ?›(<Ìa+?–yxã¨Ðq?åÏkԃP?¶Ù¡kEy4FGL J1026.2-5731¿·GÇãۑt?–Òi!ŠFôÀ9éû±¼¦À;olŸe‹@Jê½£@|<âž4?Ŗ•BÇк?æ¢~ù˜@±À"š^»@qܗð÷ú¿Þž±{¸ˆ¿é֑Ýµñ¿¾Nx^
¢E¿ç±×JÕ¿í%óìÌG¿ïÿÚÁ,/´UNASNone3FGL J1026.2-5730?mv֟LCè?ƒníÃä?ç•Ô·Ï?ÃҁñP?Ñ­èG÷Û?ýLá
½?‰ŠšÀ?1y'«l[?Ó­B8''?É<W¤9Í?åÄð¹"R7?Èï,êXÐö?§"ÔÄÇçG?Ž10žUVG?âJ^Lfßh?µŸ*¦4Ø?Øx¨Î™DG?´ÑÏXþï?å&,[?g0Õ¦"¨Ý?Ü°	ýj#)?¹8¨ \?áh0øþ•µ?¹}›4FGL J1027.4-6324?Å	3O¸¤øÀ'…‹Å›€À;¬7æ÷~À<š¿£ï]ñ@$»D;Îã?öœY~÷W?Ñ^˜¼¤áv?§C.d'®?Ó5ëŸJÞv@Ta#0†±¿ï†'_8u?äv†ºŸ¤¿ìÏ¡}éÑ?Ûq¸ß¯þ`¿á^@'—FÙ?›"£Q
AUNASNone?èPõoºq"?ÄYåéYþ?HæÛ÷Jî?D'…À:¿ö?ΣCeî¿?ÄTK£>¡?âÎênK3˜?ШǍ/øn?[dc	è?{^£%-)?ÚG
5É?БÇÉ4Ì?è§ï8*ݛ?¨o(‰E@3?ƒyÞ¥}•N?npBñM?Ì(¥4ü°A?§ñt'Óx?ëp››­r?²C=Jïm0?p4熬)?sút\
n?Á¼ßêG?²[º'Nt4FGL J1028.1-3550¿íLÉ*gø@2‰)ˆ†À;;$ŲÀ<qÀã/@àåK@ðO‹XŽ?ÀŒDœg)Z¿²ˆLj;Ýý?õ$#–=â@t#I†0Ü?ïÿ¯þ_ìпïmªÈ–g?Ò×#gäè¿îx™¿YFÃ?Ò£ƒþ&â¿ÀU\ã°¿UNASNone?ïYØO7u?«õÌ#í•?eh)V?uÎß¿×Q??Ápø&®?ªèo<—O?íG=ÀŸí¤?·×!ýWŒ?€÷ÆÔMøË?•ØË?³§ vÓÅ?¶™å]	¬?ì|•T©î?›3ÆE'q?'0L•Ì‡:?…ùá®Ý:?·ÏD·çŽÃ?˜^Á m6â?í˜Úà~î?£w–MwÖ?]ždhf?dÓ*ªm…?²ÄôßjhŒ?¢ô
è5$T4FGL J1028.4-1539¿Ú=ë?­·@Au~ºñ6À;úÀoÇÀ<vc¹ã»ý@ˆ<[Ðá/@À_@˜?ÎYßð@¿¨0ïáú±b?èu ޜØé@'
_Ä¿è!¡ÇåÝ¿ÎôK@ññ¿ì(Àéi¼¿"¿¹úô9¿çoP…S'x¿ÝݖH¬AUNASNone?î—@ñÃT¸? á%eP?a›ç+0?[׶Ÿ¦¢·?¥r2q´5? }ùp±"?ïs¿?… MRƒ|?E†·›ý?R ü¢q^?Š­*¤Í±?"‰ãq÷÷?í¸|Wɒq?•À#ñ_ޕ?{,ˆ§PŽF?j§ €g¯?°‰T·>c˜?"OF:ù(?î¤{Քr?ŒÝw!csP?nÙ(:‹Û%?ckêkÕZ÷?£Ê¼~ýû3?‹€›9&"4FGL J1029.4-0828¿êyßofÀ(@D@ۜsh­À;!KeY -À<ŽL%r€P@6;ƒd@á#=ò©Ö?¿Ïq—ÇÝO¿·Ž†@ ?õ»‡*+M@ÅCýÛ¸x¿ì!E_…¡•¿ã2¸ÿ»a•¿âc×dÖC¿á@÷A¿á¿¾¥пÄO1ÁnìUNASNone?ïK°à¤?‰Zž¦&À?gfýÙìÛã?^òG8•±?"áæP?‡©ñmˆ
`?ïSa1{ú?šΧu?Yæ1È¢?e8ü™«m¶?›ý•v¿t+?˜ÃNç)!?î('"ÁåÑ?'E\~†f_?xYù7¨ƒð?hB,5Òú?ªk§Œì'm?ž$9õq?íú¥"ÅÆ?" –˜~?oøYW®?d×°Òèà?®V(ñHÃ1?'ÇŒ'éªç4FGL J1029.9+7335¿ïŠ4ûpŠh@Cü¥aMø±À;–|tÅ¥À<ö)¢¹ @ §N}ça?úÌ
Jݐ?ß.M»tµµ?Õÿ™¾, ó?üLØç&?ûÏ?Ž
oE?ïû³ûð¿ì\šP}F¿áÃ9¦û¿µ;—Ÿˆ4Ü¿á"ÀĀοïÿÂÃ^UNASNone?ï%†ôbk?›k®<Š?g",@Dÿ<?dÑäëyC‹?˜\»ë©ÿ?šOn	¹bL?í¦#b¥V?®Xé™Â?‹÷ÞRÿwD?"½5én¼?°ƒÓŠæg?©ûw2 x?ì‹SÛ®? ³‰"Ìß?Ž~\yÿB±?³M	d'Ž?·×Œ!:3?žœôÍ.Çé?éÄæÙ9"9?«¥Ê\ãA?ëJà.?ŒplÍ'?Æé'1ØÛ?«t›!³Çé4FGL J1030.7+6118¿ïù¨.v¤¼@HBã¼ÓZ†À:pöa7À;ÐÑPÀô@>/»"zù@™……žÙ?Âc'¦b*¿¦¿$ÝHß²?çgºú<q @ÐË}í@¶?ïðL2Þ¿èò‰?.i¿éüp>–©¿×ÿÞ<`Ù_¿ïÿþªJl¿ß&|¡;N‹UNASNone?ï(ïã'¼?Ÿk…Ž÷;?"$窜²?¾"ƒǪ?Ïø§3!?—ßóŠÍ?î-«Q(þ?§_©¨‰î?~%_óðX,?,¯vÎ;?©`žñe?£õkÙ¢?ê¥ÇPþ1ç?§n¼!ÂÜ»? KiÉ·'?©†"2?ÁVa"Ê›?£þÀ/é?è«O+¸~?¬Cê–bÙ?Ÿk¦n` ?vË`ß{g?ÉeO!#R?ªÅ¯io±	4FGL J1032.0+5725?žòuÄ@I"~bÜn+À;<Uw*ÙÈÀ<†±	¢@@(²-9I"@ü¦y{ìà?ÐPP~?ª÷J=ªŸ??ÜÞÔa@·«?쥗•C¯¾¿åŸRu¿é|CG}m¿ã à_Ñ¡É¿å18‡0
Š¿ïù
By!T¿ÔcÃHê€UNASNone?ïJŸYÀå?'•ŠXssF?fÝã´æB?dG˜¥Aì?"Ðs+†&?' U<5½?ëš×š‡›y?»rã¨[?£zÙܼ=/?¯Ä«RÀÖ?¹kÖ=e¥?²Ý.ä̏|?ìía¬?˜Q7u'Ÿ?"Zg^l?ƒù=6Ôe|?³¾^t¶?"Çcá<?çš-gËø?®\.ðwÂ4?±'vµ• +? ¶ès@˜¸?ɏO°?ª¬"4Ý q4FGL J1036.3-5833e¿ïcˆ'Ø'¿Ç;»cÀ5õÆâ¨eÀ9~ƒujæ(@ ï'v"ò?þAZ=c8?"+¹äŠ%*?¢˜ÕÏTçc@ü†~3â†@H¦³2œà¿é\P˜žÇ×?ڮפJD¿Ü
Æ(Ä¿Úª¨ À€¿ãʍÜÕ¿Ø\$"ô÷ŽUNASNone2FGL J1036.4-5828c?ȵ'ý…ò?Ã@ídxÝ?Ar•çO®?H?ÉBY"?éÎ>ö`$°?ÃE¯W
[?Ý_>õ{G…?ӀôÃÞ?ŸO3n•?³Â€c'#?àUæéÑǖ?ӂºE²¥¹?Ù^úúá?³ã«8fä?¢Z§A+$w?"ÐÇ›~Ë?â+HoÝ5?´Õ¢ù?É[AQ¼e?·" £×€?›¢¢k°ð?'Â/r™÷s?èТ–}‰1?¸ÝfâÚM4FGL J1036.5-1809?ë6*üOhÀ@AÃ\á'À:Ž%ߍ™±À<^E¾P2G@^û+9À@P1ônÒ?ÂäºiÈƃ?¬Bþ'Q?æMΊ<."@<>5šÁ¿Ó¢<UpË¿å««Ÿ«y¿êJ0'|G¿æÝ´"9¼¿î~"_¦XÅ¿ïìt½—$ÊUNASNone?ï)èŸ{ù"?£šï8a?|úéÙâ?"€ðòN?""H̆W?Ÿy'3Ç^A?ïI0uCZ?'cÞj»¹?`+i\GÉ1?nDòõ,)Å?"Ô" Λ†?n¼›;Õ]?íçúhÜ1	?'Bã˜Øz†?ˆÆ•¹Ûð?x€'vña?«N´Æ)m?Â~ˆJ(ë?îíœGi.Æ?'2ãÂP?‡ì3í\Î?sštÞxž?–V]ˆãxä?{²J­j'4FGL J1036.6-4349¿ä
HÙÙó@):ïÔ8ÑÙÀ:Q-ÛÛ]‰À<Ab8Ú<!@­'¦Û÷b@CptÙÇ?À2­Ò5ÂZ?˗ä£-A,@	,辚Úâ?ý=e?tà¿Àõ5v¯_¿Þi%}½ðç¿ÛK-zâtT¿ã?Âùt7¿è¥¶ÞMþ'¿ðUNASNone3FGL J1036.4-4348?坐™_2?†™®¸‹?Á}Y{¡=?·4c¬I°«?Èd{–P?º("Tç?æ'@FsÛ¹?Åêf‰Xþ©?µà÷"'!v?²Ñc].¿(?Ìrƒ#ç€`?Ä
íèî?çÞ{<õ?¯¥£]ž©?»ÄޓøÂÑ?§¦ätßb?££Å£Ê2?¡W	Êûd"?ä_‡U}åL?¦%Ik'ž?¶Ã®'û?˜ZåqZ?ќÀt˜"ª?¥š)º*è4FGL J1037.8-5810c¿ïK4\\?Ï7äGè¡êÀ8¹Š>²Ã6À:_SUªL@±Ìp±m÷@z…\ '?ÁBL€·'?Òã%Ô¥ß@=B€®?ùÝ(¼Ü¿äÇÍ¿;Ò¿Û*«º®g1¿çƒhÀ2à}¿èeÌþJô¿ï›^?ÑQ¿ï¼~Æ.£UNASNone3FGL J1039.1-58094?'÷Ý¥n?'˺4øL"?¼Ãn/?º?çäò?ëÏÞÏñ¡Z?¼:ÁÙ‰E?"Ö¼ $ç˜?•ÌS#T?Á­Ÿ½EFã?¼1Ÿ¸Ü=ÿ?êíâ+­‡
?¼Â´Ó<Ɋ?³Ùf&7–‡?•Uë<NSî?Î}\š«åŒ?°N7-I?åå|ŽÍ?±x>62¬?y'Î5–E?fz~u؄?Ãè³æn?­S_‰%
%?êÓÎâùO?­¹''4FGL J1039.2+3258?žƒ51Ã¥@Nvߤ?åÉÀ:¯û–ä³sÀ<©J–ý'@ҏ7@.@ŽIW?ÀT;ª·#?³Ryt‹K?ð4äù}@³¨Ž?ïÃùߪu	¿ÏZ|ù$ïy¿èL%r€P¿åOàèãƒÈ¿ç|ô¢©¸¡¿ïÿ€H»ÊUNASNone?ïU¾'
?†G¢LsN?|E"ËÉ?so"½˜?ŒƒïSx‹?ìÆqós#?îߛ"H?˜õ>§<
?qO6mÉp?{(ù[èÃñ?Ÿ¸À
»}š?•ÆjåK:"?íkÚ¨_"?•€Öé?'ùòkª?'Õê‡éP?°"éF"Ó?NϢċf?í·¹Œk?'í´¤"ßâ?¥ÿ Y˜?Ž(æ(eB?žÞÐ1í\¼?€cÿ7ˆ-ú4FGL J1043.0+5316?ç!< ÿ@K[è>BZîÀ:ØâäfF†À<¶˜x1j@Ā=¨;@ˆœT?ÃO ;Ê0?Žü>:´m?Äàw9@@œ¶"‹ë¿¶ôŒÚC'â¿ãÝDÿŽk¿í2¬'ª¿ÚiVpOu¿íO|	eÚO?ÓH>Þ:KUNASNone?ï³/V? ·ßT?–ù}.Då?žˆ0j?z@'¯DŠ»?€ƒ€LÖ»?ïY>&|d?—;y´Ì?Y9"© Ý?jâ¿ôã'U?"F"¡õáj?•…ãü3*?íËèjÊd+?"
é…'ø1?"ú˜$²÷?vö'¯?®Š­P"?'òót»'n?ïÊè¹r»?j,b´REÖ?lBðvhÝ?cUJ*(s'?hÔVÜàe?YIAC)õÓ4FGL J1044.5-1439?Ô˜ýù{¾@C©~+VÀ:ãwúã`À<uMËdíÀ@qÃ/?¨@CQÞïå?ϵ»£¯?¿3çmår?ðŽ†@ €?ú¶Qô¿äß,D+©¿æg öo³¿Öe:´e¿é
¸UFƒr¿åà#¡oÑÊ¿ïäê›íUNASNone?ë¾Ò¨º³?³Õ'6?oI&ºD?iX²…$Mû?À‡ôzJä?³¬oÈ{¾Ì?î*G-wò?¤w^Ø\Á?zuF[Âô?€ð3ŽlêŒ?ªß;=‹?¢|ó"Eˆ?í<	Gxì?—ÞGªH£?>Š‰àñÓ?j+SNrÛ?²!Ç<2?"n¸Îƒî5?ìúNsþ?1OÚii?Í^>/ß;?€¨Oh‡a?ºäצh??›/Šâ¡
â4FGL J1046.7-6010?༩Ž%¿z¿îócښë©À8"k·ÞþþÀ:lµ…ˆj@9Œ‹"Y@ÕC/Ш?½Ï€±@TY?Øm©PÆÂ@ܚ )֓@MNB«Ì¿ã:©´™Ð ¿Äo-ŸËaé¿âÍQ¢4è¿ê_Á†"¿íA(¿<¿ïÿÿÊPËUNASNone3FGL J1047.3-6005?•§@†ã? ÉÿÇØ#j?çøCÐ-ïº?ÄùÝL'?Íjw7d°?ÃKtÚ¶ý?š&iŨ,?Ì¼ôË?Ú ¥¶Ç¢?ËÅfh}~'?áÞyÖnýÏ?˔<,äO?žm–Î0àL?ŽD¹òÆ?ç²Uõ þß?´&ñ"ÿ<P?ÍhõQµè{?²ª\•©Y?ƒNƀì8¾?lb3ÓB'n?ÐI[`¢L÷?°žBn¨"t?çŽ5«(¢?°¦ôÒç'4FGL J1047.2+6740?ä46+Ç?U@F­…ƒb°À;xTFŸÀ=å‡ó@ y¨ä^˜?ü'Dc_–?ÉXOwa‹`?¸.çI$â
?ðêÜ0@	LG²òA¿í$¼B;
ó¿áÁƒ(yF¿Þ€žÐe3¿â@¬ÞDïH?˜·G.%5¿êq=Å]lÃUNASNone?ïÈ¡ƒ'
¤?›QÛ¢¯?3ïÛßã"d?5BžÿZbÝ?zp@xü{ø?%€†B
 ?ï­y€•Ðå?"'õMlÝ?4v#¼@"‹?GÆ4€L]?ƒýÁä?ƒþDŸÔ&?î)µUfÉ?—ɜ¿ð?iâ«ïÏ2O?lùѤDcÃ?«Æê¡pG?—?ù€á?ïǂÒ3‰?hTÝÜ4?,楺½[?(n 'Ø0y?{Wa¸ÐZ?h7¬B(©Ø4FGL J1048.4-5030?àe¢ïX½Ü@èϦ›áÀ;~‡Å[¿À<€"Œê^®@"ží'`A3?÷&Lëk…?Ùޘ§+R"?Ò¹Ù« ê@•‰ïØj@@7Ӏñ¿Ó@LyË¿ài}Èâ¿ä§ü~Y®¿äHxÌE¿èè\૦â¿éMŠ'$‡õUNASNone?ݤp-;?ÅÒS\b€?'­Mî÷Ñ?‡Ÿ^H+×-?à ]€œ$?ÅßÌkÌ?Ï.¯-=ú}?Åvj<•L?¥y¹ÂJuü?±ýLë"?æܸ˜‹Ú?œóñUx·?èL—ë:?¨|Î9
Mz?£p+ߝa?‹×Ó$v"ž?ÊՕ[0?¥ÿB$Â?ږ߀œ?Àýè—œ7?¤mˆO=7?©>E>6NX?ám·»#O?Ã\1=úw4FGL J1048.5-5923?ØÚç¡S;*¿ÅU€e-À8µýawÀ:Œd×-©@Ì22Yò@9fâ?¿äð/'ŠÞ?à€`b–M4@èîkƒÙ?øœ¤Z诿ݫ^ʐ²¿áa%Ie¤ ¿×ÐfíÖÞ¿êS恩¸Ì¿ïÿÞý¦ßR?ïùT_}¾óUNASNone?ñÅÕç.Z?v¾	~'x?ìÂbdÅ¢?¶ªO‰£"?µ°{jZ?´èý>©Fœ?"ƒ:kp,?  YK]?ÜO¬6û^ò?Ђ
Z]AÍ?á?Ê®õ?ÐXÁ}=aŒ? ôà‡	?.o©š÷I?çu³Ä!M?±í-ù"¢:?Íî¹-6¬?°†€0‹´(?]ó—)£+s?N‡;9×?ÛÏÓo÷ðã?¾–ƒ§?â	|o5ù?½ùÀ»Oš´4FGL J1049.8+2741¿ì݈À>°%@O‰\Rç-¡À;$jÈ˶LÀ<ÂÉø6{@Èey+ü@c'†Wv?Á?wd:'"¿ª†»›w_?ê_
Awn¡@Qu=™¿?ï¤nß±¬¿é£=òÔÉ¿át€Û\²ˆ¿ÞCO
)N®¿èê¢5Ié?i…ÖüíUNASNone?îŽÄЃ-?¡Û'~??x ‰°É3?o圥î©?¤¡Á´å? û'Z ú?ïXõÏB ?˜Çô—Љ®?`ō )ð?lDMWM±8?|/¢‰/?—Yœâ""?íåécÝÁ?"žu]Kñ
?~Ü·RûÒ?p®ŠÓSJz?­ÅÐċ?'™ÞuZÊÒ?îDËPs¢?0þb€c?ƒ5[Ú8Ó?pé6ü ¢,?¦åôAáö?‹¸ï£(4FGL J1049.9-3658?àùØþ@3ÒóÂÚۃÀ;o…j7¬?À<½¯€‹¬@ü<'UÓ?þ#Ÿý`éO?×îS/Qý?Õ<캨ÝÚ?þs™õßëŽ@nÏ[rl"¿Îˆ""ꐭ¿ì6J	8æ?áO܁u¶f¿âÉ­"K¡¿¿Úû¯cZm_¿ïý_ ÷ÇLUNASNone?î'.êf8?°¿fš3v?}&¿A«¡?¯4?«7¸9qg?¯ÁT,ä½?î£7,5¾?¡u»Êùà?qµjU(3N?Is«~œ×?£•ßõ'¬?žåÆV|pG?ì_¦ðU=
? ÁjÞ Ï:?•ÖMÎ?"_KCLm?·Bjd?…ÿyPR1?íӆâçÞ/?"ªÆü׫?fYÊ0*w?`¿½¬?°°ú—@5.?"U®¾åz4FGL J1054.0-5938?ìøFŸezG¿´ê}6âjÀ:*&¨«À;zKìgœÇ@¥ðj
à¯@DÍ$
¡D?Ò=Äòø6?ÛFuš¶Ð@	Ž"ü¡¦®?ÿ[Fo¦/¿â¿°"—ª¿ààŠï²ªã¿ã ¢Bµ‡¿àýT‰Å@¿ì¯¹"<¿ðUNASNone?µ;rÒUC?©ý¥ûÎÉà?¨îŒùsÉ0?¥Ï%ñÆ?ëɨÖ?²o¯
7sú?·p~|¬»?±Vxì¶Q»?¢>80êÏ?¦š'¬i>"?ëîªáÀ‹?µ‰«äô³?È Ë=NàJ?¤ûòçuÕ¡?È8ÕóoC?¥²Ó`ò†,?ãé—ìïl?¬z«™F?ÆVÄ&T6 ?¥€MxÃ?³Vs™?Ÿ©øÉÓ¨p?çÿ€"wÐ'?«nY(Å4FGL J1054.7-6008c?ï«D«-–¿ßt_ƒVRÀ9>¡ò-¯fÀ:ºôƒÊû;@ ¬ÿ"Ë(³@#éÁЈ?Åß¼™Ï?´}áWHfK?ôc@\¢@x•±'™¿é–:‰hÊ?î6êx´G¿ëB‹`òË¿á…!ýÖ¯û¿äw'¯c¿éÎf*…UNASNone3FGL J1054.7-60064?¿9­ÉbÐ?´Ü'Å¿xh?"]"6¾?—¾-àöÂZ?ëuòHß-?·=8ò=þ?–±©§5å?ÀMš±™?™¡–}u?­Y¾î¸7/?êFáFÞ?Á;¨¨ú?ÄæçlE·-?¢ØžÛÍ·?´t7ûä?œØ8[Nœ?èDï²?§R˳µZ½?Ê+fEüá?¨û‡Kè/?£fic¹˜?'©"v%=?è>ؐ2çG?«)VDË|4FGL J1055.6-0719¿Ú'IÚI?@FË  ôØÀ:Òs«ÉGÀ<}4#;z@öõtŒ?úfÉèì¾?呈pSO?ãè›)¼'ì?ýR0",J@"B)›.ð?ï¸;Ÿé?¿á jÓ¿Þ*¤ ¿í·¬ª–¿ïêԟ©þí¿ïýÁÆßMUNASNone?ë|c '?¼ÿïù¯ÀT?'ùn^­#?"ˆª²ù?ÀÞژår?¼€PÙþÕ?ëóŒ.Eč?¾KۗFŠ¯?¡Kj?=E5?°+ˆnx@:?·½én38ó?´dH¢†Ÿ•?èÔT ï‰Á?§HkJm4•?³7˜éfn¡?™Z6,Ù?Ã㎡©?¢%:=E£?ëEC#N€?±u"`]?ŠG`2úŠ?• €"CĚ?ÁIŸyo–W?¯Ð<6·¹ù4FGL J1055.7+1033?ïߘýp^@M¶0©8À;mv"Û·À<·þ^?Px@L)ÿ'׋@Õ`EK?Îú0³&2š?Šæ
²ûj?¸åõåZ¸@xއ_ZY?ë;>À<{¿ê©p§2'?²zò9˜Ó¿áöRš™Ê¿àsø^K¿ï—m¿öûuUNASNone?ï=™ZŸ#"? ÒE'Oo?FøÙx5rV?WýÇÝN?—•
àYáÛ? Nñƒ¸ß?ïbØ8ru?—¥î¾&ÎS?JcÙá'X?]÷Ö{6Í?'ÑÚ)ê?–ÕŒKzre?í§•"H¶å?sN£ØÔ?s*TdĜ
?l9XbÓªä?±±§mÿ?œ¢Ò£3é±?ïg9|ÔÜ?{àʈÞ²?RîQ+9ƒ?IÚ¨Jé?'éëUyä?{%>áÚäw4FGL J1055.7-1807¿äs*D!B@Bb¢"ÕÀ;†PÎN­À<¦üZYê@`àëgÃ@T"\Böö?Å
{"Üß¿·Y ¾Í–Ý?óUE¬²{@'óÒö­?ï'S‰êÏí¿ìîbHŸ¿áé€C‡>¿ã")Zl] ¿ÏfD˜
xT¿Í^;I­UNASNone?íiÙAé½?ªÏ®Å"ÝY?'Er²äm?z‡Vƒü«ƒ?´üǚU‡?©ˆ'éx¤Þ?î_ó1ØE?¦EÌÝDã?w4(rú¤?‰Î[â@t?§GÔ=|b?¢šr3/Z?í@ÊNÐu÷?˜îöâ5t?€¢ZæÍæ{?qBy¦hÈÚ?³åb,¢"x?–~6ž·ã?ìÂQjàu?¡7ӑövK?r>ÛÙ??n0œ¢¢$È?¸É"A¸j? åÙ@Ús4FGL J1057.6-4051¿×÷ZP@1«\9¼ºÀ;T'ÏR¹
À<¯ík¨Å‡@!Å.	¹?÷ÏY­€?ÕÛt/|ÅM?×­ãænß@®¤Ã™Gd@ЈÐº%¿ïÿóÀ¬ƒ?ïÿÿ&¦³?Üe·>ñŠ?œÖƒb~-
¿Þqá">éu¿ãJ½Y<\UNASNone3FGL J1057.6-4051?益ތYÇ?ƒc£¨yM?U—½Yó?RVXfË~?ƒ'±Å?'–w
U?ïf¡DÐ?™²È¶Ä°?TÜރòä?l:˜…aCï?'Þ	•FÜ;?—Œò
m­?ímL{vs?›3¯€`Þ?…G?ˆ'?~FՋ¢?±ï
«$…?™7uáñà?¹TÜ5?}j¶?eˆ&ðHÛ?Y'VƒÒž?¥üñû­®î?´³ÖV4FGL J1058.4-6625¿ïQØMŖßÀú†×6&À:©ˆúååÀ<@—ŸÄV@ –|¨È?þÄâ½ÏÙÈ?Â%;8eL5?µ¦?piu?öóFc'ŸÐ@à¦ÉWø:¿ä|Wisa?ïò±}»í¿æŒ"ÎX¾¿Ò¤e¥vF®¿æ,SzÑWv¿ÙÞ¾‰¾UNASNone2FGL J1058.7-6621?ì8?™øìì?¯hÞOlÁ?vú֚å1?~óùµä?¼ÎUƗ
T?®æÇi¦.?ãŽÞ'ãø?ÇeXRâV?h—ÏØÜ,?yïgK\'?ر=4
X?ÇIZс`z?èšñþq˜®?¦Ÿ)e©³?•¢
̈́`?}‹‰£¹‹?Êó#Äßì¸?¥z'È	?êJ[‰Êº? ¼öD2šÜ?¡H°ü,S'?ˆñ~Ç?"e™Ê#?Ÿ˜-hlGÔ4FGL J1058.9-6101?èZh'º¿ñ"ӟNå@À9¢G«<#À;$•%–'~@…¿9fS@÷xmži?Êðmü1ê3?ԘL½rç©@™È î!±?÷ê–߀Å¿ïÿ¸8º1?ïøVˆ¢ÑQ¿à2Û>Õ}Ë¿ã<æp–¿ï—_'œ}?жƒ_E‹UNASNone3FGL J1058.5-6106c?¨iB-õsE?¼oEøö|?¹Ð÷±L~
?µç± ¸v?ë?Læ÷
?ÁKˆßlD?ª®n—z?¥óv‡€þ#?Å-HÄñK?ÀuŒ_4?éRçÚ5#?ÀŘ<Â@?¿DRÂä€L?™Ýêƒ^œ	?ÉUÉ•ø?¨ÕóàBÓw?åÂ5uaÊy?«LGe(?´¢oeßì?•-Zf0R?Ð]Cë±gÉ?²q­MA¥?å="P?²zZºë¸"4FGL J1059.4+2148?Í!ñ;ý…@P,{‰
ZÀ;N1‰åÇpÀ<•ÀY÷Ã@ddàÕBg@îà¹Ü?З¶€G7?¹d
ý´÷?èñ'?_‡?ìKV^~ª¿Òn¡¾/•¿ã­`öºÝ¿âл¿^OA¿éšº–icq¿Ê÷‡‹z¿ïñd "‰UNASNone?ó‰?ªžW%K?sXð²1ì?|²OG?™?¬Šå"±)ƒ?©ªé7¤H?ì'&î¹³h?·Ê_0K¬Ü?š"¸BYß?¦ÏI_–?´ñcœ!Î;?²2îi"$?í;a‹³Ã(?˜ û)^²?o
n[?"n›u1ºŠ?²wTû]?"[°×?ç9ª‰œ7?°jóNy;î? Š·'л?—¡ó2ø_?Ï`ku%Œ3?°!Ž1á›4FGL J1059.4+0226?ë]R	HdY@JɏÙý7À9ÞkÑà2À;òhÒQq@‡séèw@½‡Ý¯s ?ÄåýJn
O?Á9ul"§?öÿ\‰ÉB@I¡yŒÞË?ïÎ` ©®¿ßè©¢%YV¿ßÙ=ˆ÷Šæ¿ãX{Â=ä¿ë²‰ŠWÝ7¿ÞAÜCbU`UNASNone3FGL J1059.3+0224?ëÂ´˜sƒ?Ä8¶w?§—û	!bó?Ä*ԑ'–ö?¶#œÖ«²m?°([¡9zÏ?ï΂Jº?•°E€ž©?h'n<øj?t(뎨Sª?šZ˜h›a?'õЁߠ"?ëïŠì¾ö+?¤íº?Ÿ»‰'ÑZ?'i­h1?¸"Æ5TÑ? §|´ž?ìŒEQ®*?•DÖvPŠ«?›±\8N?'½¼Ã?´±"›€›È?'
€¢ù"4FGL J1100.0-2044?ëù£æµ½M@A‡´€¥¬ÍÀ:ÁçIOÕ*À<"÷z€Ï@@¸žÂx`@SÕ4z[?ÆÆl ¾4?¼C"Ó†û1?ñu~æ­?÷µ×8XŒ¿Õé4 G3¿ãgšx
ÿ¿Ùsÿ*¿åÑG@~š¿ãæàtI~¿é¼«aÃ'UNASNone3FGL J1100.2-2044?î
PMd?¡üÔ`Ò}?mO¶S%½?d·vÕ.ù×?­†U÷Ü(?¡¬ÔSÑ?îE*^æ:? ó_c6}?|ߔÁÆ?&ƒ¯ô?¨*>&?£b1'"Y?íð¦•Ýí?•fU·šø?‹@tbؒ?@GˆEdí?°ˆl>õþ\?'g™­˜ÁJ?ì'bB‡WÐ?—Q8êbÌ?šýT£@8S?…Sâ}à'?´­˜Âõ3q?"´^D;e4FGL J1102.3+6715?íÙ/<Q @GJ²BÀ;è¤nòÀ=0fC*÷û@!PØ?ɵ?ûV³»ƒÏ-?ÏAÖçØÂ?¶î•ÊW&­?êö5çB™Ù@ÓLÙ!™Ù¿ï¥íÀ7h!¿Ô°oó ?ïù0¾
í)¿æ{›¢|K?¸Ï2ؚ`¿é8%@+i:UNASNone?ï×O¹/C3?s¼…N¸¬?&Pk,>?$c`AǽG?s£¸å?sO™Gì?ïyÀ¹¦£?–å8
Ö%Z?G…úÞoø?bRʐøÕ?¹·²Ð?•Æmüž?í>žbâSÝ? "$7>«?|<M^æC²?~<ã;0a?´GHþüÛ?Ÿ*ÑÍn?ïÈ#÷ôF?oij(=…?%ç̸%:
?,%Z-!£?{>Å Õ ?o0ø¿*Z4FGL J1105.1-2600?®éœ·kç@?â2ŸÀ:ŸÀgnÀ<'•=†Æ@'ñ§Lµ@(í½\ì?Пª?ÂpŽHÌ^?óå3E§©þ@ÛÃ_»§a¿àÕd¶býü¿æ6ü¡%Ôü¿Û"ɾO†{¿ã/ýÍpa¿ïÿoì÷å¿ë¡;NŠ§ŽUNASNone?í¬[¯²—l?¦ÊoÌþ˜?v­}a-?pŒ"&'«=?±;÷ª›'?¦'ªBžÌt?ï5g‰>ó?"!«íїZ?auƒ?\?p[èüÖø?—$jßîÙÃ?'>'~3–t?ìã"I×s?›y²y®E£?—ÄHp·Mª?‰}+yE¤?²öÑAƒq?•Åî×k‰¡?î‰+?ˆ;@ EÀå?€?~ÇSü?qDa"µG—?£]nÖ2g¹?…n9‰ô"î4FGL J1105.3-0626¿ã¾7šdßl@Gß÷øʂÀ;¢HÕ[èÀ<´Ãð…8º@#P׿ïï'?³k=¯:@?çµ+ÆWh?ïÿKÚÉå'@""†âÞ?þ¾+õ&]¿ïúìšÈmÂ?ïØQ?¸§§¿ØŸ½J"ä¿êèD§¯Ý?æÑò¦{)l¿Í¶¥CÃUNASNone?íتlš´?³I®~êœ?ïSðSdí?',˜¼ý31?©ý¯Eü¢P?±{9AÇ1F?íÇ«	?»Oë~y<?'N®Tá¢?¨^ÿÂWô—?²ŽFÇ{?µÕ6»#¹³?êV̘uâN?ªô¶JˆD«?§ù@Nl?"º	•­?ÀäONï+?¨
ƌ\ðS?âþqYwxB?ÆlÆê¡x®?J½†'$Co?jñ0Q?Ùõ¾‰È}[?Ær2Z{Y4FGL J1106.2+7303?ሁŠÈà@DüM:'£À;þ#qõÀ<5‹¶'@'Ÿ‹¡y@ãÏ¥Å!?Å^BÀïÉÒ¿»'¹5Á-?õÀ´á¼©@«'â[?×}_*ÝÏ¿ë3™àf\«¿í~ÞAê05¿—'n¯¿é[Ŏ*Y¿ïæöäÎKRUNASNone?ï
þ9¶?ž,
l‡[?Še°í‹?‰@F÷Œçr?'zËh0ҁ?˜#Y£é'?ï Â%ù? ^øÔrÃò?k«dy*;?=
¬»êF?˜‰….±¨º?˜K™{F5X?ìãØ^ß&ö?šYpsË?Œìªª"ٛ?~ŸtkÝ?µC§³Âm?—²™û)Õ?î¨@î¯b?–åóJ‰"º?"Ô[ªiÃ?"
žÿg? Fü**om?'ácìYqƒ4FGL J1106.7+3623?·mTþ³D~@PŠ\å´$À:|ƃÝo²À<]˽Ù@ø³"כ]@îwÐÛ?Áq56î~£?¡Œ ?ƒ¬%?ÞwÒ>Nš@m«ÿøž?ïÿÎa¢\a¿àÏÜKÅÑ0¿æ÷ôގÁ#¿âÝ­Å ˆ¡¿èך@]".¿ïþ!nÑTUNASNone?ïåeÛÒd?'᝗¯ä?K•?hÊj?xå2kã,Æ?c´ÔSìê%?‰ab‡Hã?ï³kk¼þÏ?"H\ë|1?<<X'Ž¯?Psâxý¶E?'CBL+×Á?ƒl…}˜?ïátíÜ?ƒy«J«	°?nýÉlNð?]|¹.¡<?›AñĔº'?÷xd`~?ïÄhR…?dŽ…"Û½?WÑ[Põ€˜?DŖÿdi?wüu(]"?bîùå?‡É4FGL J1106.7-1742?îv;NÆȸ@C=À~à±À:xø‹—xWÀ<†]Ötì@‰ú‡;?þë'*ç?Ãì[!Ý?Ùh$¬‡³@pÀ\|@Í¥u«¿æ¤;~[O²¿¥~ŸBP©¿Ö¼ð¡=Qð¿äó;Ì_¿ìƒlfZ§ì¿ðUNASNone3FGL J1106.6-1744?ãFe3Ž¼D?Å@-øWß?Òöq¸ªT˜?ē|ulûO?¹ó€à˃?°_ˆ1€?év³àÚ±b?Ãi"SÀ'`?¸õ³§3M?½n0Þð9?»T­RA¡?²§lR¤?Ðú·t'R¨?µÏáü…"ã?âKc²Ó?¹¼wÃ?ÄÞ5	ld?¤|ß~Ÿ ?éôÓdî×î?£S8íÛ?·PÝï'Üù?œÚÌy÷ƒ?¹†écž?—~áêf¹Þ4FGL J1109.1-4853¿îëãÚ@¹ë@%8ñ,'¦7À:eÒ(V`_À<,"d®ÖB@ˆ¿¬¨À@Ùýñ7?Ϥ4<ȈE?àãm"BJ@€˜@Ô¦@lLJ±T ¿Ê˜ÊÔпÀ'/Cå]¿âz•ÈSÁ¿â*þ~ð¿ïڋÒ0¹Ü?욉¹QÅÅUNASNone?كÈK¸?Äþ("ù¾?̤JU	C4?Ápð¶?Ø*¿
z®?Ũæ‡å¤½?äÆ <ƒ?Êãn7¯¦º?Ã@žýCq?Á¢—C'	ì?ɦàù̒?Ãj"-ý+?áaÌa/«?±ЬvG˜?ÈdZƒÄœ?¦ƒ,ȕô?Ñ
9ûñRª?ª9]ôV:Ü?ãèqӚ }?±öCä²àì?¾Ó(ð&ˆy?¤}Œ¨Ì=2?ÐzRÁç?®77"x±.4FGL J1109.4-6115e¿Ø,"{Wí°¿èÑØ8såÀ7C9+À9ãKÁŸr@!ÿr:Uf?þÝí¡Xª¼?£&"S¼ì?¦¯
šÜ@@Sý®(?òIK :?îT­×>?׿à'°+¬V5¿ßc? (ÿԿۛ㪵¿ãÍ®oê¿ÚpMû‹| UNASNone3FGL J1111.9-6038?š•Z7.SB?…È:eÇ?uB}o!?{h5vpù.?ïÑ
K¯#? m¼ŠÓ ?ˆ¢ 2·(N?™.+â횂?Ƶ3.tþì?ÅÖD6"?éð(³—ã¤?Å͛]'Ð?±vOüŸs¦?›‡ï€ÚA?¦ô¬e?'^|E{?ìaë?;›9?¡q•Å˜¢¯?mp-̺-ú?`&ôÁÇÑX?º†?ʒß?¦Á4lêŸ?ì'ÇØàó¶?¦ïË(kü‰4FGL J1109.8+4406¿ïÿ¸R@O»\6À:À@æzýÀ<±*_Oð@WŸ
ÌÇC@ñ¦Ö˜þi?Äá~_¬bõ?°¥¸¶ÀF?ä»[áF×?ù¹99²~B?ì‡À=È7'¿ç"y߿éÅEŸFÅ¿î!çEôÖ׿ïÿµ¿Ö̯›Ž'SUNASNone?盧©£•?²JªÝ0!%?`øK¿?il£Ô¶¼@?'•ÒÓK3?²Hʓ(e§?ëq{N›?¾¼Ï¼|?«e'Kò´?³£¯°òI~?¹{Y²ÿ'Õ?³l¡K섓?큖_ ?˜mC	Ôû?'heG§U?"tm_u?³eŠ¡c>ª?•{Ö	䧰?ë>D'µz?ª{å¤"Al?ºe"_xª?©l£ó¨?¦àò[ée¦?ÜJ͵à4FGL J1110.4-8023¿ïxz'9ËJÀ2aA…ÞÀ;k‰lû«ÝÀ<°±¤RZ@@!ŽUºF¸K?ó¹Ef;ž<?ÛÀÚ»¢ØÝ?éöh§‰Fe@"å$²fð@2¾/%1"¿ïÎ8<‡oË¿ísXHÕ\¿åš\!¾ì?ïgõbLM¿Ô1©ñb¿ïÿæŸÜ©ºUNASNone?îþýÊy½?žƒì¡€+S?9t+
JF?|lÚÀ?˜Qé¦Ëm?›ükÊ+7?íÎ
ˆǙ?¹`Ÿ¡Y؟?‰FŒÔú­ý?¤ðz+¾Ì?¬Í"I"Úó?µÕK@öÙM?ìv"ÒÆ?¡m´@Ȋ?'äS"¬X"?…œ;V!?·Ò'>¹B?ž¥¹1žã*?êْ¼!n®?¶rBƒ?cø?'²ü(/˜?"õª=T?Ãp¹ß·ÂO?¶,"³WÂ4FGL J1111.4+0137¿á<Sy5X@K€`VìÕÀ;'‹®ŒÀ<bjáö)½@û}9f©@XdàTi?ÊÍG›õêR¿=ugÓQ_ê?˜ã#¶V5?ùðrƒÖ
é?ïîtÝw"â¿ëqBb{[¿è&Ï!»¼"¿ÔÈUÚ'(c¿ç–Háñ!@¿ïù&A³(·UNASNone?ïxe"Ô?ŒF…'¼Ä?[Ύá¨ä?U@Ñø¢ï?ŽlÉ^
d?‹!ÚÆ,)?î*:öAD?¤éÛì £Y?w»dÐ;æ?~ãuæ¼_?ªfÿ¶"n÷?£†Çë‰4U?íc×ûÍ?—	ë}	©?"ÑÐ̆@T?tkœ6áú?²M'&—‰?"±¸x†õ?ê׺왮?¢:Ÿy1?š£ë9-¶?…Ã1Çˌ?Á_Ð2"?¡GJ§>Ãt4FGL J1112.0+1021?Ô#?ò©€@N›‰
Z[–À:²˜ˆøa¦À<beÀN9I@ž¡@W@	z¾A?ÈlxÏ¿®•ûÝå©?×¥_ yˆ?ÿã&«esø¿ÝÏI~Ïø¿éu¢¿<_¿ïaß¹8›R¿ë"ãw3=D?ì.rýMž¿ïÿÒ³–šâUNASNone3FGL J1112.1+1034?ïuЉöäw?–›ž_}Õ?}üDcºü×?¾ ÍíD?ƒ»Picá?‹Ûä,¯è?ï$ànü¨?§º˜•æ[§?pû—×-×®?˜ÌLZì7-?—%H"õ?ŸÀq¼ßÑ»?ìâ y);N?˜ù)ßaÊÅ?ÚE‰:'ô?ƒ%U¢¨?´ï³…ŽÓR?–ñ€•¸?ïÞ
¿Îƒ ?o|Vs?5†úMû@'?C"ÅìX+?oD`ç¼ø"?n<&^·P4FGL J1112.2-6055¿áVqKN'¿Õ8;SéÀ8¤à·e\{À:)1™Õÿ{@ 
y#ŒÈ@­'hr°!?ʚ_,
u?ÓOW xEŒ@T>S!æ?úyLò÷ÙÁ¿îg8¿d?¿ãÎ_ã¯+¿Ôv§ý	«z¿æ¿£ƒþ&â¿éR½g)/¿ï+4+€·KUNASNone3FGL J1111.9-6058?x'ª"°)]?p¼J²aEÀ?Ãr¤»|Ï?À*ÂÌ/;ã?ëÀ‹Ày?ÀYô–Èr?Œü'ûl¦?'±²4$ÿ|?Ãçÿ:Ü?¿,¹DÛj?ê͎L C—?¿ŒÛS?©èr'Õ¡ã?ŒÜ¿G­º?É
o
kO?©<r*Z?èçä?ª4,þÑ[??gŒÅÃ"?Säñ&˜ò…?¿lkªw?§™lÇ·ð¡?ëúñ"‡ø®?§"y8|™Ê4FGL J1114.6+1225¿çi¢Ñ%Ìî@O}Ëݹ"À;dÑ~uYÀ<›ç+ä<@g}ÕÃÁ`?ôFâ!ȧ¤?àþ'î?ïÿqÐ&ô@Ø®$kT@I§¾ËW?ï<m¿ ;à¿î»+à-§®?Òa¼­ž¿Ö‡KMÜ+å¿ïÿójÆGx?ä"e}2ZÆUNASNone?í×É`]?¯Da…ÑS€?"`O8)1?", ®%?¨ÓBj'ºw?ª@)Ft??ꚧ¾¬sR?Â
E
$Ô+?®x1t.«ù?·DéÛT#?»î©P…w?·ý‡A¬¯?ê'ûx5?¦©ô|×S?¬e³¾'A?–N7i)ö_?À GJo‡j?¢›óO?åå­]j×
?½+¯8Î?šªö2û"Ð?˜ùnÓcëP?҉õáú™š?½àÖCÎññ4FGL J1115.1-6118¿ëˆñŒ}Z¿â-tw¡!MÀ8D~ïÊ'×À:
ž¿s@ rHqß@Öº;А§?³¾R`Ÿýâ?ª‹~g¨Ê?ùãòhgÈf@"³U?ìŠ@Ë¢*b¿ãÆ
`:Ó;¿ẩæž/+¿ç'¼£n¿ä˜êýºU|¿à5몥çUNASNone1FGL J1115.2-6124c?°ÿP§"¢?¡áø¦CÀ²?¬Š‹‹Òc¾?«'`r:b?ìm2REu?²‰Ò‹‰·?¦"d\õ»x?¥t$:_¿?Ÿ&fö?£}觞Ó?힉¥l™?­ÀÊ£¼¥¬?¼þ"ãhVq? 2šf:?´l…Ös ;?™ê™¤
"©?éÒªèā+?¤†"õúô`?©ŸI<œß?¿…%Áß=?°sõ%¡6Â?"ñÞ?ƒB?ìWæ¸Z?šÕûß½4FGL J1119.9-1007?Ü:tw˜ŠG@GQµc#»ÇÀ:ë浬×À<b¢Œ‡b@N-ۅw?ÿX×1ª?Ñ+û›í0ð?΁ûWϟ»?üöË #÷@	^0;;X?¼äaئä¿ëY:>b¹¿Ã;Û"zÿ%¿á¦ßîÁ¿èRàýÜ9Q¿ïÛ`í*»UNASNone?ïFo¿ð?"ã­ó·˜ë?dK­^Çé?`g·¸&&ð?ší¼\>cu?"ýsÔ:X¼?ïOs^+P?'¦­…#7?Ry¶ó"?`tVñ:?"êeM?'ºå%Í?îŸFƒÑ¤?'§m²ûB5?€Ø‡}G5 ?tM§Cîo}?ªé¸qP?ÃÀ?3@?îƞÿ'$'?ƒt/ ¸Âš?j&îLm¸?WqKÚiG?¡ó¡"-`?'»î÷k‹4FGL J1120.0-2204?ïûÅØ´.@B(ÂzÀ8Ígi›¥
À<ø¨ê@Þ}˜19´?üæ+ÈÛ¦"?«µÊ|»gu?Þäµ—&"@/êjP
@•'æxðW?ïùÙ?¡Ö¿¶UŒ_°zî¿Ý£¦ï¿è"kdÒè¿ïÿûbâMh¿ïæó{?UNASNone3FGL J1119.9-2204?ÂsPÕ~?ÂH+ˆØÛ?êA;›(?Åꅩ2¼?¢";Þù?¦7ø4Êü?"*¶zåŸÁ?ª £
Ç??îi}òHS1?´¦Y'?Ÿ¥‹<ú*?¥ssÖ,?´…gÁº¾Õ?¡žRt'?éÙ`ÔÃ	?¨ã1äNë´?¼¯'˜,Xã?¢¢t"'f&?]KŠ¯ø"×?WÆÕºÆU?îå08Ñ÷?T$º¼,D? Â )l?`å1('4FGL J1120.1-2645¿è}w$#Ì@?Ï>$þ½
À:GXS~,VÀ<_'fÅ0÷@÷´Lù,ý?þèõÝgNÄ?º/÷¿i·Õ?ƒlßHǼd?ÊaÁ'ýö@­¨ñ{Wå¿Ù‹Q¢Š$¿ã5æzyC¿Ü팈†w¿ßœ7£Û;û¿â6þ™Îs¿«P'	ÚoUNASNone3FGL J1119.8-2647?ïÀßnP
?pƒT+ғG?I:B?<ßg"ªç?|oá´µò˜?o]?^~í?﫜g/±?ÜÀÞ3XH?=…Dµ©?Mkš ¤Œ,?"/ê
&<?o«gyN?ï˜×.¢%?jUÉ'ÿ=?f
Žž!?Sü¡·%U†?›Ë3W7÷H?€KN»ƒE?ïê¸|¦Ó?} [_'M?^˜`?ge?H9÷w??›–jg/7?|ë(šªÈ4FGL J1122.0-0231?ì.·+¶ù7@J¬wFˆzÀ:õQ³PúÄÀ<Cb?8È@Šx•½ìà@c줩(?½É¹ÇâWN¿»é\`º;6@k:á}]ú@ܨX¤0÷¿å•b'¬K¿å6fœí¿èð«Ï&C¿åé'yâ¿äû9âyÝ<?Ö¶›Ø'UNASNone?îô½©<Ëì?¡î€˜9c`?€ug&zæ+?{%Á"*?™-—E)?¡&£B‹ö?íÇIº
N?³ù"8G?‹ ¬ÿ'ÿ?¨8x>ìn¶?¬Ê‡Izo?ª<ÎÜ!!?í;—ˆÄW?˜Þ²5öL?Žtc"Þ_?&–.n/?²T³Íj«¿?"Öh¤øo?ë´ª-¸ët?¨Ÿ2°,e?‰¿&ø®kŸ?'ÞYaÄ?¿"ɳ"Öï?§@}¿ª7w4FGL J1122.2+3926¿äçaââҌ@PðváÞ¬ÉÀ;(à#Á¦(À<'i<Ú{â@#³—œ"@[iQ;?Çúj"2°¿¡C!£ú׳?ÖQå&µÌ?ü¾#çÈe?Ö_#Æ®¦¿é¢²G‰
¿çXl"h	Õ¿åþ‰¾]¿éPKý"z¤¿ÓUG¥[ÕUNASNone?îK¯:ä{?§‡ŽN•4ç?"©áØÍq?‡‰"
?¦–f["û?¥Ëê'O¸?îUQÁ·½?§DÖqxD?ww÷¯B¯?…gEÐÐ?§»ä?¥/µD:$?íj9š
?•
ŒÇºìt?Œ>)¼Ÿ$`?}Pkfhß?±&møs?'§­â7?î7ÒYã?'cìÐê¾0?Œ}ãØz?{®·6v¨±?¨½?5­?‹âàõ¤u4FGL J1122.4-6237¿ç¹]¤Jø¿ø"ÊL¿ÌÀ9SdžJÀ;
¸ÜU
@ 7~ä6¡@Z¨!ò™?¾ònGx? ÜñC_âO?æ)Ïqºû@I4ý7Σ?î²:zOQw?ïàß¤jٿ媚rÝm.¿èÇ)Š=D¿ÍÀ‡Y¦¿ë	c@—ëUNASNone?Òf3ø{»?À/›p)rN?¡ö篃?¢8ƒ@DÀC?å­w'Gƒj?Á3NLØ?Ð.BñУ?ÅÄÒo¤)?xrÇ5ÔX?ŠÆÁ%ED?ç¸Nø¬?Å­ÑB;YÀ?Òª¶L`³Ë?°]ºÊV`?³XcŽ
*s?˜Üö &Ž1?ä?˜hÍ?°c{=ZJ"?ÙÂfߧ
?³É0°z¶¦?ž¼ˆjŸÂœ?'‰™Ç?â(è°;.e?³÷ûßôƒ™4FGL J1122.5-1440¿íÁНòl@Ezã`'À:‡ànj@æÀ<N&äpX@Þ2>k @|ÿŸ‡ð?Â|ãUzZå?°Bü>l?çu	Ar;1@ꖧ 볿ãOµqfu¿âøÈÔÈ(¿é=ß>ir4¿ìåþÌú6¿ÄçxŸ£ô¼¿Öԓj«o…UNASNone?î Gh9?©öäeµ™ô?"Ôí)gÃf?…«pjÉØ?¨ÆRį‹Œ?§'ñº¢«f?îJÃëçëi?«|˪ª?u,‹äÔß?"g_T)ZB?¨®/ÄæÇì?©3MB}ü?í&ß6êr)?•Ä3@è?ŽÛçzj›?€UÁ{ž
?²í‰Y_T?'OÖØÊ}?îGc•é?'fÜAOsA?uõïÑwT?n‡g>Á£ÿ?¨ì»Ìrq?'"}Ú»•/4FGL J1123.2-5111?ïרcó@"š{9&À:¸ÕŸeæÀ<RÂ&@»¡iÍf@NeÙx¬º?θ©?Ñ&?×8´|sîå@·±ÚØÿ
?ü|h±D[¿ïuH¡¯g·?ïé$ò'Ð)¿àL"b¥¼"¿à2kݞ¬(¿é4èªxäî¿ïÿŒ	ß}UNASNone?ç<ýZæj?¾ú7Fõë_?žg¿Â­î?"3™è8;@?Ï?'üoh–?¾@Ó·Î$š?å4_‰£ç?Ɋ§ԀÅ?´·+m8þ
?¶#&œõ:?Ðiwžx°?Æ´Ž^«î?挞,?Ñô?«éãä74?´}@0/+?šn­†`÷?ˎç6é+š?¥Ýé\cçt?çcÀPx.A?¦Û{èè×?ºé«ê¾3? ŠzfÍ¥?Äüzh)çç?¡aÕ©~4FGL J1123.8-4552¿²¶1¹bA&@,­kD¸ÃÀ:2ϾÕÀ<Hóµnâ6@Œ¾A™¨]@ÜOÜ·%œ?»Ýظ¾M?±g?Õ-'?õ/$*³Ê@qI^BÖi?ïùJYPԿʓÂjU%¿è-YŸ®†'¿à×ewS´¿áÙ[ñ˜^0¿ì"Áœm	UNASNone3FGL J1123.6-4558?íÒV#Oh?¤Ó¼¶žy?ràªít]Ï?e¨ŒèöU?°?EH>Ù?¤e¤Ö¢Ü?îÒÃ㥍?¢O+cõM¿?bÒg¾ïƒ<?wcªëþ'?¡¦§•Ö¯?¡8'áò`?íjH"å??™f‹ësœ?…v;{n l?sQÿµ°?²®Këî?–æ{2öµC?í¸ÔiSçì?‡;W?'U"OOu`?u¹þÄ/½¹?«G÷CƓ?"4§W
Ø4FGL J1124.1-1203?ŠN÷`ÿ\@FºY!…ÆÀ;+Ÿ'xÀ<•®Ðbƒƒ@Vï|úýb?ÿ!ƒ†Ý?Ü­$ÜtÏ?ä¶öq@"恩¸Ì@ïZÎy¿ïü!~|?ïÜ^o÷ß ¿Ù€¬ã£S¿éCa(¹Þ¿î-‰Û¶tœ¿î¤Q]똕UNASNone?ì2§ÝÞo?²ÇB !A ?£pQAË2? vÒTò?´áˆèk¢?°e]ò‡L¡?ì&®˜7V?·Å)쓊?¡$ĝo¡?¥!1ñÇW~?¶<üðï}?±pP!Ü?ê~æWê&?¥"çxŒ g?°$ï×ûñÑ?—°¿ç":?»ãÝh²ÝT?žJËèLCK?êäöšù»?¦`z"¨?©ô0ÖêŽB?žÀ†öÒ֖?»å¿ß²ë?¡Á7X|@4FGL J1125.2+2557¿à…˜¦yk@Q­LD|0ÓÀ:+·=ïOÀ<€¼ÈrÊù@Ùÿ°yÛ@ð@|ÇÑ»?ÄàðZÆu?ÕÁ~gô@	¶§[ùûÚ@rZûÏ×?ïýË<©Ôz¿æ	g½~{0¿é–¹èîl¿ê""½¿ïý²GæHŸ¿ÓО¥2UNASNone?ïv5•#R?'ÿš`Ñ?†ugŠÔÑå?Œ,ŸEê8?x	IJí?{!3µÒç?é2£hñ?ÅcöØ·Ëh?¼XLÕ?ÁgA×Ë.>?ºÏÖ«Û¦?³`#%ù;?ë­b½G5?¥ä
d:ÂV?«¢©G~)?—ƒŒÿJ–5?¹¡@FV±Ê? 	Ôám?èlMesÌÉ?­DvÕ-Љ?Æž-«Êµ?¬Q/'›á5?®$0òž?"¦Ó¦dï4FGL J1126.0-5007?j``@$ìܨââ¹À;E²à'|oÀ=–"TÛú@˜Õ1 6?ÿoB]r¡Þ?Ó|
}é?ïG}½›¢@ÇVO—î?ý)ºËÃ?ïû²}ì¿æ5‰2C¿È'MÅ°£Ì¿ÒՖŸê³¿ïþÂ^§U¿æU/þËMUNASNone3FGL J1126.8-5001?Ýë¢ã¿î?Ë{aby]?×Ǭy'ö.?ÉJM¥\kZ?ÆdÏÇ2"Ì?Á]þrÛÕñ?°/_Å&i?ºˆn¶iî?çVK#•v¤?Êöò(šéu?ʏ#ïG'A?Æb<±÷s?ÒJc'|Ræ?²+¨Õ¼
*?á&¶»,?Ç?´¬˜Bÿ´Ö?ÆÐ^ÄV[?¥Ç ŽEß%?°d<ü;!?¡‰ëN1;Œ?ë%zÝÉ)?²Û_B€a?¶oì{²'?©¼lq»T¢4FGL J1127.9-6158¿Û;_¾Ú.¿åÁ¹óêHÀ8ÿÁõuüÀ:²ÿ%¿­@Òg°"[<@–øAŝ.?ÁÇHhújj?֚ɚh@ߧÃ(]?þk§ùÈ.?ãů¢›¿Û–­@•ql¿ã×ómJ†¿éå9àÌ^¿ì¼í[¸{¿ïòÌ&°nUNASNone?"uÝ¥û3?‰>á=F"¿?ÏñÈ©?Á¼H€Ÿ?çhG ¥æ?ÁþǨ©Mz? È§êz'?œŠÈhÞH?À5ÑØ÷ý?¶Å—$êÜ?êæLâß?¶êQÐ!I´?±-Mÿ{ö?·¡'°<?×2×®?µÚÝ7ÃyŠ?âV–·wh?µEåtÞ?†;-6ûJ?mïu-'?Í/l=–>?¨Q¾A',}?è[8<}œƒ?¨¡ï1†"d4FGL J1129.1-5230?ÂüÖ#|u¶@ ´Ž:!dÀ:ËêpKÂvÀ<BW¿¶n@/§J\D¤@#Êŋì?ÁÊZÒbä¿¢E›ÚUe?áKÌQ|ÊV@
ájCÒ ?é|=}¹ê¿ÃJ&¿²]
¿ê……t¿Ù-Aª‹¿ßEqcÅwC¿ãñ" Ü.UNASNone?î<×4o? àÌOñÏß?a°¥Hý?Y$†|š?=?«.°á®³? ªx ì?ëEhˆºKÆ?Á«ÙÏ[0?QÚ/'Ð$Š?rX25Ì£ß?ÂÆ©}ó0 ?ÁŒ^xI?웆Ó!­?˜‰X$ãÚ?}쫇Á?kµ=X>Ƴ?¹Dþµf‡?œ'ÝDPÅ?ï(?}Œþø?}n¦þ‹?W^ÄÐjlV?H‰øÓß?™'$YzH?|ÕlÅí\ˆ4FGL J1130.5+1400?ÏŒBn¦@PÁå!WhÀ:È£öꭈÀ<r5r
	@a
þw¥@îùûA?Äm¦ß'm?jF/Ä{µý? ÕÇóE:@ýClç4¿å¾¬#¿æƒŠT'¿åGxÏõv9¿è|üÀZxœ¿éÒŠÝ>4¿ïmè jUNASNone?擄"îc?ƒ™¼j¤j?UC6êVx?Pçv_(h?"+tu§{?'¤«yV?ï˜:Y!aÃ?ˆ/@ǝG?D¯ÐðòÝé?V´Ü‹a;?ˆ¦l¨˜al?‡¹-ûR4?îËÂx™!?ˆM8C涟?p«¸v2\ù?aÙڊNŠ?¡.ag§ÂV?†‰è³eéÉ?ïZ늩|?q×'#£n?cô¹u]¶Ñ?S‡ƒ‡#ûÇ?†ì¿þ3A?p{þ¤:
4FGL J1132.1-1448?ëMߏzº@EgÀ:÷nªØ†>À<ræY¶U@ #3ºÂ‰'@¸ù±1f?ÐB¬©—?¼¶ðÂuZö?ñ åRՏê@3¹ˆw]Z?¤àA@{?ÒD4¢Éî÷¿å.â q¶¿Ñ²;{+¿ßö'þ¢ˆ¿ïþù:!EUNASNone?ï¢t]KÈ?€hRó»Zô?HxÄ"Ë?P¬çh7èà?…Û\jì«?~–Kí'?ï¢uÞؘó?"öòÆ\–?A9q—a–Í?O³~ôK?†Nñ0c©æ?"4ll[?Îß?‹ÎÚèÅ?i߄ÃP?WIöí?¤ ÁUß#?Šv^xi>?îãŒ*Œº?ƒÍwl_ù?l§ñb͇?\ƒ²hkó?Ÿù|'NNã?''½d=Åä4FGL J1138.4-3555¿å(ìD%7·@8¥à?pXÀ:Ì<Ý ·À<{(7V®b@ؽ›×a@Bý@27?ÐâÛ¬äz?Ó(.rýN@ä%C†gŽ@`'ÿ÷q'¿åív% Jù?ïý»ýœ£d¿âRÞt?¿âw8¡Jr¿ïú?–më¿ïÔ. §TîUNASNone?ïÒ\{ìX?"²Ƀ®?€Ð½Gðh"?zû	\7$h?•}Ů@º?I5ÉòÐU?îŧ ìE'? y"1Ç÷X?|±C»•×?ŒQ¤»²?1? ]'5&?™G‹ØZ?ì[s?c"?Ÿÿ–Q@Ò?£R]áÆÓW?ú쒔7?³}åu!z5?–š5Òþ!*?í>åÐÝ×ç?"+Üöâ>F?Ÿ­*Ÿàò?ˆ ‰€Ê)?¬;
¢•?Ž¤iÅÀ4FGL J1139.2-6247?ëÇY5¸¿ñt¢iKôÀ8†8<‡oËÀ:¿mã2ià@uòœj.r@¸*Ž;?²î	!U©ï?È3<mn˜d@þ¼ž_ç?üQº¥WèÊ¿î¬B®Ûö?ì"ß(#½¿â†¢F†¿áë,i–¿éH§8¾o¿ïþç àö%UNASNone?¶+.ð?°fs´Á?܏UVbú#?ƞ$ºÈÙR?Ýåã¢Ñ'â?Æ ¿ ÷Yâ?£Ï.ƒf?§dº™`Tü?Û~¢Nrˆ?̽dŠn?á½%ކ?Ë%<ƒö?Àë·?Õ?¤mh¹Ž€?Ñ;Ü­Ù?±Pr¹Ð?ã'$9C}?²øýju!?¥®ðU÷"å?Š¬Û-Åc¼?Õfð»'?¶'ÃM1~G?ä]ì()é?·q4Øï/4FGL J1146.0-0638?àŸÿ¾D@JZ?>pÎÀ:b=ç™À<M·½q7@!'Æ¿¬?ùð'Iü?½³TUª?½`OKÔ®?ý\ÄÞÁÂ?þï·]yÙ¿ïý?Æ¿l'?ïAJ·æ¿´|£ÿùõп;«·ShÞ¿Ø-‹¾åƒ}¿ÜŠ"¾@BUNASNone3FGL J1146.1-0640?ïf%ÏB'?‰û_X°÷?`A¬.z¸?WÝl3\èÛ?')]â'Þü?ˆºùə¥Ë?ï6x\9?•ì·eŒV&?e¿p÷³U?q™Œ$'CŒ?–çf]Be?"eHgQø?íqh2_f?–Gh€?€j
Ì6:6?pc²táØä?²g|³€E…?"Š!ʳ4'?ìäˆ!YE?šAÁghv?–ÝÖ
¢?'+šœ~ºT?¹Ú¤Iqñ5?˜ZˆMÁ£4FGL J1146.0-6822¿¯IMñfÿÀ
[>ê÷ZÀ:lF"
qÀ;Àê×yÎù@¾§ðõK@W^ FÇe?ØÖrÓ\3?Õ'H㞠@¿ìTR@ã´2!:b¿ïûì?XÛc?ïÿ©Î›&¿è0Ç}Øró¿â±ŸŒ¨¿ï䍞8º²¿ïÉ™"{UUNASNone?ܵa{u?Ċlþ}--?¶ÍG¼??°ÂÀ|;H»?ÞEø¾Á{?Äëِ7<?ԋ¥'9=R?Å>ôr{Ue?JZ(Å®?£?©h¨?äÏÚe8z?ÅNëü¸ª4?ÛÆ"%"+?°¤¡åy©B?ÃßÐ*Mþ?£"èæ½b†?ÚJVÏ6Ö?­Ôçù7.?áú6àåÁ?®nŒ¤<LM?­æt'òtœ? ÌŽ
›Õ?ØNíבé?¯›pÊ4FGL J1147.7-6618?ÒV¨/Àê^ ŸGYÀ9ì¸ô¨´À;{oɼw@ÖÙ¶?A´@…æÿ}ú?ÌÞÏÄ#?Ò6Á}cX@-F|¼A@ç;¸è¿?椔3ÿ
?êÉTýÞ<·¿å'ÊÞ
6æ¿èæRkÞ¿í¡]¹»¿ïüL·h·yUNASNone	?¼>ž§¿	¶?­Ž¡·#}?Áy˜êL5?¸¥ý@ç?èÅðu;?¾¿Ù¯"½?Å·NÂT‰?·á:p¢Pï?¸ýêíg­?¸
>ãȂ°?çþÔΫ½ç?Á\͊Ûq5?Èõìrc?¦–í¼¶úI?Â?«£¿T?ŸÄß"3Ÿ?å2ԛìNa?«]S}Ï?ÍA€õ;Yy?¤Xžµ9
=?ÓAÈP;*7?²6WÊê7û?Þw5')?¯X\‹6
4FGL J1148.2-0029?ɛ»žãA@M<=îx@À;+&ø'MuÀ<‡·ôÎs–@֛3w¦«@BúP"–J?ÆHàÙôþo¿˜à>ˆk?Ñt¶`NÊ=@€èÚ™ô?Æâ=¢Lñu¿Ý"PÄé~‰¿ßÃ!R`¿çúy
2ª¿á\ ý¦‰l¿ïÿå]½JyUNASNone?îµR'ULß?¡2$`d…?t&&¼_¯%?iU¥e$—?¢&<5? ÔOÁÎaÉ?ï­>ß?—»#àõ ?^ˆ&B¼?f¹‰Óéëë?žöß°?–«éšh
ô?íKºP™?"PZÔOêú?ŒŽ2ʃxÙ?~Ňl܊Ï?¯ç·¨Uº?Æðåöê?î ˜ì,/?Ž	/ê¨?€*l]"²?qºw@3?©ëÖ'¬n?Œ0]Ý)ž4FGL J1150.1-6324?属SpH¿õy€TN5îÀ9·Lz,	À:öðf/	@:Ïzüö`@_¤?åÉ?φbЋž?³Ì{O,8?ð_zNz·V?úH'ëÕ|¿îóÑôSúS?îc2Õ?b¿ãå˜u­+G¿ìbXŸÔF>¿ÛÈFøã¿Ò…(€nzUNASNone?ÇA—òýƒ¢?»çÂç¢-?†œòµ
C#?ƒ"òv-,?éÕ&8lj
?¼²aFŽ> ?ä9äÐÞÙ?¼äFlNà?§H­ÝÕ?œ£Oñår?ꑹ"†Y\?½TKôgæ?ÇÆgßÎ&?¥+NóÅ?´N5˜ŸÆ?—Y˜Q%ö?焥Yiþ?§Bõ¿¸'c?Ï]"Yä?­2Â*c?M÷?£¿?'N‹}?çSxáBÐò?®æz3$Ñ©4FGL J1150.7-4613¿ïñVÁ¥Ô@.ºp6ÉÁÀ:†Æ÷ µîÀ<i´g{9\@›Ö_ȓ@"i7Ñþ?Â&Œš?¸[GàzÏ?÷êg²–À¡?ú%[Øï?ïôÿ¼
aè¿åÊsbοãîð®Se¿Ýñ^|¿åƒ^)+¿ïÿÅbu@UNASNone?îƧxV?¦J*Á‹?Y?to¥P5
-? OCgq?¡{+Ù]?Ÿ	¿¤±'·?é KRc=9?»Üö±úß? DÑ®ú?¢*X¾é?ÅmÍB-ß]?Á}úEßï?í8	?:ށ?˜'> ?ˆ%fÛ©?uÄ?¯Ë¢"?³;	*ÅöÓ?–
*I?8?ç­'¸˜F?¢le±…Ú?³Å(zn«!?•‡3hhg]?ÉÖµ{æIZ? ™O7ËÓ4FGL J1150.8-1905?âÄÅö2f@DÁâCV—À;Çj
_ÕSÀ<Ýû@ý @"B;ë¾'?õò…=Ân?Ùõð"?Þ¥*ÜÍuê@Ðkæ'ø?ù	E0‹¹¿ïÿ+YJ1?ï)·¿Ža¿ï±	b¦é?ïþmÄ(¹]¿å¥;X›¢ˆ¿ÚD÷€Õ}uUNASNone?ï^#jOބ?'rq	â½?m-'	*?sŒì@ýÿ?•ât£Ý?'ñb2²?î&2ñLŪ?´´
(œÝÊ?"@yÉ?«Çæ­F\?£ü"c&ÀÛ?¥Á¥‡!4?ìz²"jEô?¡ p$9Y×?'j$SFvá?ƒµ Yî_¯?·âOÜ2ª?žUç‡k½?êÌÁÊKA?·R
»r_M?«RíIø—?²™È<±ï~?¼H7÷J?¯ç´üHÜ4FGL J1153.7+1857¿îAÞÀ¦_@R›ÓíR~RÀ;QÓq+¼FÀ<¦?|ÑÔ@\GŠ®@²9{Kй?Òx‰éù-~?Ãyç!·µ¹?ñJÀ²¤@Gz½áM¿ïÿ*LÚ¤&?ïâ¤.™p¿á¯ÊÈæŽ?¿âzó¼$ÞÝ¿ë6#það5¿ïÍ	žs`UNASNone?îÃgLG«å?Ÿø}|Fû`?wI?‡]?sñBáÚcØ? àcJ¢6?Þu+–Å$?ïp3";Ñ?ïÙ|cC?UŠÞh솨?f…âØçÏï?¦ë¨é½?ŽžJk-_?íA'ìÚ?œªŠxÎ]?"o*ê?…[çcnû?³(­øè4?–ç|¬¹ ?î"cª
¾?Š£b¤÷½?"ž
#W§ø?t›Oê;lÖ?¡¢BÖ9:-?‡[4ý0_Ì4FGL J1154.5-5952?ë']
¥¨ú@ÀµgUy¯À9ۅèÜÎÀ;gcRµ¯@íp¨‰¡@¶*ä°a?Ê«r«fÌ?ÞÅè¬ý#­@Â¥Fv@Ñ)÷öP?ïÿ«|,Ò¿ß¼ R:Š¿æ3ªïê¿í'›h¦²‡¿äϵù¿ïQ(l/ÔUNASNone?Ä\r€Æô'?»±3	yp–?°å¾´'pç?¬ôy®Ô™?èÌ+‰=ôÙ?À	Ó³ëñ?Ñá ýNªù?Í΅†¶ÚÑ?½ÏEKý?½~øn?ã_gp?Ηo…
?Ó!º¢åÚÃ?®†&ü?ÃÙyBZ?¥wE@ªTR?á©àx.Â?°Ð£ü"Ã?ÍJ÷µºš?¦,Ò«uH?ÆCr¿lŽ?ªa†ŠÄú¬?ãebáKö?®³ˆžÎò4FGL J1155.2-1111?ÕOÇÿï @Hª›(ÂÀ;	)ÿ­ËÀ<ˆ‹y¢ƒ@!õäs2?øRñ>œ?ÜXiwÿk?ÔaæÕw–?ù‰,£Ìù@lƒ¼7©:?Æ5èDL‹?í•9î8W_¿âãeூº¿Ð`LpñÛ¿ÝÓ]ÀOâ¿æßÛÒú
xUNASNone3FGL J1155.3-1112?î->'õ?¡]¡­þ]·?…wOÕ͟)?†\^¥àe?§ÎJb]G5?ž´=C²?ïKóˆD1?'­ù{Lä?ZіlÜ!??hÊlœ
Ã?"Ôu¯÷Û?ÿž×1ž?í
«<À÷-?žPPFïø?‡²"Æ"´?uäšz
¬—?´œaÕÿ'B?›ƒì" Ù2?í!õœ	{?—¹÷š¶?}ÇQ?xO0ø È	?µ1'¢¢Ù?—OŽbÉF4FGL J1157.7-6327¿¸Þ8P›§P¿óQÚ7ïZ–À8ô".E©À:•,oʓ7@>8?6¡¨@ÏKaþ!Ù?ɔš×1T·?֊MÌ;­U@áã!¢ç÷@÷ÚE±:?ìÚã{dû,?½ê2S¿ç×Tz«—É¿ëb)ösD¿îBýûÈä¿ðUNASNone?£߸3l?¸ŒHã+I?Ù[ù­†	?ÊNý1æ3ý?Ý­´*8ñB?Éfá ¹(?ª©…0‰óû?§À)')?ÅâïžæN?À(R/­?é®ñ§-?Á
ød?ÀÝL¤É
? ´=j‰?ÐŽ*,ð¹?¬ýLÁ}?ãô—ÀU`?°Qvy>¼?•¡¬™Ù®?y—:ü§êl?ÒijpK?©"ä‡uj?æE¨ã²?¨è¦Ê;2b4FGL J1158.8-1430?îº;h@G:‰ãC0×À;ÊNmK]À<}ª?K@!ˆ~7éPf?þ±ÞŸ]'ù?ÁŸ¡EŠx¿¿®å;µg?ïèÞ%d¾?í·«^×À‹?Ô}ÖÅt÷?|¹H­æ$.¿èqԞ}Y¿æ(ŠbÄñ¿Ê"Î×Ë®¿…Ôª'¹{aUNASNone?îq(ìµ?¥êXQ<ß?pé¨M#B?w9réÚq?¦Ð<4¬àF?¥.!r£!ø?ë¬Eìú$!?Ày‰H2¥?¥÷Rp?µþ;±ÕšÊ?·¢M…ÝÅ?´u‰ËÃÍ?íEÑ
%$×?–Øt%˜ù?‡6±K`^?~¾ðÖa¯?²ê¡Œmm4?•})ÂÍv?ß:ǟÿ³R?¶­&.1	?®·³FÙÏ?§µ
ƒPÇ?ÜîA÷%+4?º(pÑbÊ»4FGL J1202.9+5818¿ï™ä[ùj@L×z_A®÷À;'bþÒÙVÀ<½·ªü˜l@(¶o\@HÿÚpú?ÄÙ»G¿1Y¿›Ï(¿`n?Ñs×þ")ñ@òà¦ÉX?ïøÀÛýÂ8¿ãÚ¥hõX¿éfòH‡X¿îQ•	ÖC?äp@¥½£¿êÚýç÷ËUNASNone?ïæ+L%Ð?qU¿j3Ýá?E7¼ñáw?TÜFwÅ
?d—ðĝ·š?m;ãɂ£?ï0~n®ì?ž¿›Mp-?bŸ*¿é~±?{äúuš"%?—œLä,ò©?šÄ"¤›Jr?í kf¹?'ù>ZÝ-?'Z¦à!6s?vg¿eÙ¥—?°°2à £e?'CúÝ}Q?ï̜O~If?o.ˆÍ½?7L㚀!?A®"œP?x=¡¤É?n"IŠ,4FGL J1203.4-6145¿Ùˆ#:Ò*?âé*ÁI¶ØÀ9ƒ×Ð6
ÙÀ:Ñ;§uû/@àúãe@Y~™cõ?ËPk'kSá?Ú=Z¾è]¢@½C^#¡Æ@VÒõÜ?ïÿ9œf¿äӟNå@¿åuWСm£¿êUŒáû2¿ïÿÕ%t.¿íýØ=CWnUNASNone?ÎH•°º?½'y'†AÅ?Á$Éç?¹çý¥°ð?ä$ÙN‰?Ã×Ëß·/Þ?£­—®"µ?¤@äwÑeB?­ßÎü°ïU?­©;øÐT?ìç)•L°¯?±v‹ï?ÂR#þ­d`? ²¶jhZ?Éð;#gÇÏ?©C§fg¾Ë?äïh7z´ô?¬ñ°ñל/?':ûL}ͺ?xV-!'Ü?Ãڀ±&?¤•€ÜìÝ®?êw‡ùVH?¤µÒq¢0«4FGL J1203.5-1748¿ÖXþ¢'x@E˺Ü	€²À:d&°mñÀ<gÍ0ŸÚü@ý}}":7@…±ã<zÛ?Ȩ|¶^÷1?Ðӛ=]®‡@{ÜpêN@jlU\(¿î³zK¹?ïzV¨ƒAi¿âÍg'ߐõ¿âÁa~õÿK¿î'(]í¿ïÿ•AED®UNASNone3FGL J1203.9-1745?çrõiG`?½M(ˀ@›?¸¿™Ñš	Ë?°C™"¬5?ÅÔ]rzØ?·¦i•'­?ê(TØ|¡É?Á¡ªŠZ…?³Í´ï7ˆq?¸ZµPÑ?ºï¤LãiE?²Ø€:¸?奎+T?±+ú¡ È?ÀšÜØž?£(¬â0?ÈÎë9Ë?§È`'ML0?ç.x‡×ï}?ª¾êŒóäC?ÄÀ^PN¦?¨l›žªT?½ ¤fÑ?šNkö4½4FGL J1203.5-5745?ÔR"¢jÑ@"!Š"CÀ:˜Ž:À;Ö©n"óJ@aÎQ1@ ;êŠ?ÛÓuþ‰Þ;?àÈðÔéÑÀ@YcˆÕý?ü%͌Fµ?ïøÕ~Í"?Þ0×Cÿ¿çcvÇÝyÿé·R²T{'¿ïýðƧÞ?ïâÆ3U—âUNASNone?á$<¤3?ÆóÚ{ž~ƒ?ÒNÿ"×B?ÅÛ	H•åb?ÇoåÁ"®?ÀbŸ¸Lç?Å8^ÕÙä?®Ò¥îÉ?ÒC—¡¾Ó?ÊЛcB2Ê?á¦Æ~¸Û?ÊRE}ŽÌ?ÙÁ؛ƕü?®¦1ä_ŸB?Ë%Ùå`¿|?©Ä+Qyœ?Ø«:q‰
F?®¡|E8¢Ú?ÂiŸ÷ƒ×?¨"Ù	ì?Øõ-Yº
?ė([Óø?Þ
žª"
?ÂîÞ
½Q4FGL J1203.9-6242¿ã
ôu濛¿Õ£òfa´À7럓®žÀ:ƒÝ ×æÜ@åÈøן@lû@}ž'?«uPºÃú?Õå@Ìxé÷@(0ítA@ÁÊqRӍ?îc'ŸÐ¿Õ†šË'¿áW›ÝÁ'°¿æHiü¿ìòFñ'¿ïÿúVrÓ\UNASNone3FGL J1203.9-6243?r°<µ<ìš?m¦.‰¸3À?î)¡Ñ@ß?ª:E'n?«çLDT?¨â´àèHI?wY$ك,Ù?€V´UNé?è—	ôBC,?Ã4pæÙí?Ìé*Ùé?Âì*¿C'¤?‡hIa?{ ;Pa¢?ì¸QUd|C?Ÿ1ºïÏbí?·Pl(¸Ùú?œGÌþ7Ð?C	&A¢?5_;/0?ä÷¨^âú¤?°†òQ÷Ï?Ö =sw˜?°'¯:È4FGL J1204.3-6111¿Ù'©ŠtÛ?ò¬š'^ÛÀ9Ù¨g'¶QÀ;(Ag©]@úhýoî@悀x`?ԐY—Œy?àœ<ÁÒGá@
ƒn´é?þÀøãÖÿ?ß{ûú?ƒ`MŒiŸ¿çÒ(ÁÀ)P¿í[ˆêዿè.]@L÷*¿ïÿÖDDÓoUNASNone?¹'–þՏb?°g‰šu.@?Á±ßëL‰?À.×ûgœ?èc5%R+Î?Ã3!KSš?±æ]ìë'?µ
lŽ©ß!?º>Æöƒw?»Î"Ø¿'?ê{[cŸm?ÀÀoX^*?Ä!ÿD`?¡Žy'J±µ?Ưj&à?«Ø!^J?åM].È*?¯²!k '›?›në  _i?€5Èô®){?ÆC§ùR[°?­Ô!ž#?铞¤ªf?¬Àøm4FGL J1204.5-5032?ïó±'eí½@'Eík¨Å‡À:]4=õ.À<ˆ໗@æKùӖ@œ…Ý$3?Æ4¸Œ£è?èΙ«7@ Ù#¯2@cLÝ(d£?ïìQ'(¹³¿Ô–)ÂÇt¿ÉôuˆBYA¿è_[5z`¿ïùΝ²X¿ïí¦–Ø:UNASNone?¾­N8ŸBî?·6¨v×dÑ?錬,³u?Àï慈?´íPg3!q?°õûbúñ?¢æ»Vw8ã?¬Oغ£Q?ëh½¬õ¶-?Àa]zW¨L?»F´í²)?ºýCÿS¼?†yLêÍ7?¨‰›Ô£?ç
D‰ëº?®Mn§[·	?ÁDt‹fJ}?¡€¦ò;ô?³7¨"õŽ9?—ÔèæÎD?êj""¹=c?©¾2ø4í?¹t37@†¯?¢Ÿ6¬4FGL J1205.1-5951¿ÐJ¼O.Äí@ü¢¢&0À:1š‰ƒ¡áÀ;œz'
‹@°†ðõv@…õ'^éš?Ç7ªÉlÆ?ª3¤r:¯ÿ?漺Ñ!Æ#@‹9&A³¿âîO~mnB?ïøYþyC¿èˆV{6Ø¿â­RH¢0A¿í/†ÖHv'?Òja}ss?UNASNone?Åþ/Eéiþ?Á¤›•iÆA?£4VYçÑG?£'PðtË?éM.Èç(m?ÂÒø•2G?Ý偭£$¡?É
ÃÛ|C;?—Ì d¶?¤±¡_™¥?àNÞ(]ªŠ?È÷c;ψ?×6ݏ2?±&Ž×1åû?³еs¢­?"]ÑZ(ÒV?â—_
?°šy/›L?ä'÷ýs2?ªÒ¹ª(ñ?¤ƒÁ'G"d?'µC6ŠÏ?ÕM7ë'/?ªúbhœ4FGL J1206.8-6038c¿âF`‰O
?ü4xã@¬˜À9ÌAƆbÀ;%ÿÜđ•@Êæ¼7(`@.ùèŽÊ?ÐÒíÌw?Ï`Š™ÌoZ@¹5v'\@qæOx?ì¿-b
翱ɫ/C9'¿èöĝSb~¿ä¶‡æ鯿ð?ﶞaUNASNone ?ރ]‡ñî?Äù}>C«X?Åу)ŽÚh?¼a<}'?֔9
° ß?ĸ~Gpö?Ä|x±<ËT?Â˯68?ÁÊø¦ÑF?ÂD×üsSç?æ€o‡Ù?É"Þjeî"?ÎÞvIŒ?¨(…ð²f¾?Â坳•Ù…?£Ý‹1×?ãŒÛ|÷;?«æ´¼³"?·3/Ï•ù?œCÞdF?ªoZÚiu?¯íªš¡?ènþ5rã?±WQåõP4FGL J1206.8-5836¿ÐiÈCƒÀó@…`&±EÀ:»™ž¢À;ØA'è|V@ê×yÎù@I¥ë·sŸ?ÕÙ*ÞÐÛO?é›ü_âhÀ@¥º9LR@YCNa?ïôáÙú2¿ß1É~X¿å~®@ð‹¿ï!ÃÔֆŠ¿Õ=ŠÅ@fx¿ïþÿðÇôUNASNone	?åbr2#‡¬?Ç0P;c¥*?³ñ pL=?²Î©þÀf?Ð>Ó"Ý™?ÄsÈëÉ?ӎ×t+ÁZ?Ê^´k€¦?Á½™ãU?Ã42'ÀÔG?áÉ.ñIì?Êä9æFO?â×ÆõÞ?°1ÂÛg?ÀÊ»ÖAv?¤h;)/]?Ñëoê)#6?ª‡ó*b;"?Ö¬æôM"?²B'T+I^?¿ŸÇ«hj?±([µ¶hÉ?ൔ")?´þ¿Y*]€4FGL J1207.4-1840?큮¶Ó;@E}NÂò®À;@Ë]a'À<˜Šï²ªã@'¢ivç?þ¦êjl…d?ÓÒÆáÑ@Ð?ВôÏJU?ýkؖ.«@(*…È¿ïüþX`f?ïü1©Æ7‡¿ÙÓåŐ¿æ{°&äp¿ÙÿÛíÒ¿ïÿõEq#UNASNone?ïÞÐÁxG;?pFcá´½)?E5.x$H?Eó3¤Þ?káúüº¶?l˜æ¸t"?ïwIÞiPº?Ž<)2X¾o?P]Ñ.?`ÃîAO¢Å?òRh×p?‹÷'ö;w?íÑöÝ®Ï?'ØQÐ†?‰›õ¿wH?{"ý²,úk?¬™ë'®E9?"%"Ô?îáí&/ç?†JDÕvð?ià,H0Nh?`ñ©ú|á? C+™ü°?…{±.D84FGL J1207.4-4536?í͂ù*_
@0"süPHÀ:tŽ·¾GÏÀ<}MPëªÞ@`Tßd?ÿ<¼æ¥¼?Æt~A¤e%?á7^3'þ@#¥ ¶Xí?ñš0Å´Ö?ïÛi³"Ü¿Úï
Kšˆ¿ÎÊ.·Îbú¿æŒ x°ì¿ïÿ
A1"¸?ÊĦ}ìUNASNone3FGL J1207.6-4537?Џ–'…J?½°2Æ?ã^6ª
ÐN?É ²ÙÓä_?ÁgøS¿´6?»3ÑG´¾²?´ÉÓ¤º1?¾SЙ£¦?é,B'?ÈÜÇ¢·úG?¾´ÊG<¸?¿šÈÀVR?¹ãb(µhs?Ÿr(º´C:?瀏?­Û[ÖÅá?Å£)KŠ?¥Í9ùÑ?º´u&œl?Ÿ¿@֍ò?åü"sL_…?³îŠ#ˆ!?ʵlø;3´?®`"Œ'4FGL J1207.9-6443c¿ï¬ÍKDCÀþ}~°àÀ9ÃÚ#Íd¢À;@+ôzÀ@ü¦¬| @ÍG`ç¡d?ǎ¾^9ò?Û`–ƒ9°Ñ@"yJ@«"6‹­H?ï#BÅwmö¿Ý}M¾NÚ¯¿á~@Ï~¿åOãm"BJ¿ïÿþÞ÷?íkP`j£ãUNASNone$?±ËPS‡¨?¥ÃõÐáµò?ÆùnÁ·'‡?À£IÕE²·?è:E!R‰?Á­(Þ<x?ÂfCºÜ"?¿Õƒã¢",?­³.œÐÏs?°ùx¤ž©j?é‹<'{êf?Á4¶êÀP?Àï"AñOÃ?¡®x²^Ú?Ò1™âs°?±ïö¬vó?â¾b'r7?±·‡S‡GÍ?ºÚ&$²"Z?£,øå
¾(?¼qŽ9–´?¦ï8Åqº2?é‰t1ZŸ?°–	²<{4FGL J1208.0-6900¿êŒ"+ëmÀÖ¢?ZˆãÀ9ú¦wÎm·À<åaïa@*AþR*ð@âÛ,!?À9­å×?×ù%ò-/@ÅJ]ò#ž?ü«?#VqQ¿í¯/˜sÿ¬?ßÑ%ʟ¿à¬ÅZèƒâ¿å'¹ñ·é¿ïÿí¡Ā?é7"^6UNASNone3FGL J1208.0-6901?´Ðqçù?¨†·¹æ/?Üb&*3çŠ?ɼÙʋÉÚ?ޘ%¹R?Èy+'·ü?»‰íÉ$ÉÓ?¾xÄòòm?Ú[P}ýzq?Μdt¸ª?ÞÂ4¹S?Î+#<J"×?¶©–r›#?>ITè2?æ‹U§µÿ?±hé˜	??ÌEŸ'Ús?«,èdÎ?ÓhH"Si?°îgq"²'?×[i%rV?¶z6¼M?Õ<	G:A?²ñíêÙ
w4FGL J1208.2+1158¿ïó%§Œÿá@QñŠ '§À;<n—OßÀ<·;÷ýÒÿ@¡è:@g¸Õ¥¹?л›nÛÖ?ÃsÞt$?óèÚI@E¹F]1‰?³õ¯o烿Þà#`"*¿æîÉp!¿Ó(ËÑ$J¿ïÿÿ" 5•?ïÿú@ùDzUNASNone?ïaN%=é?ž‹?±ß¿­?\~¡š¢ÏH?a¤õœü"?'ì!®Ó?ž1
0?ï
ç¥l?ž
Sªb?eÓ›íß?t~uXƒ™?œ~H§þþ¶?›ôÊ®ñk!?í¥"¨Îˆ‡?•íB€Û[è?…_»Ê]V\?x"mŠKh?°*ó@@ø?"©GP?î­õDÿŠò?Æ3"é>D?v[ÄR$È8?kø<úìä?¢U3%·Ü?‹ÒØî{4FGL J1208.5-5512?¶¯'«ù@­\œ¹À:Š÷mŠGÀ<'8Yã¡%@×XìÖ-@¥Ò! c¸?О#y+æ?Ö½±[­$ç@P—\¨wƒ?þýîþOü˜?îç%pÔ)¿ßg"ÄËL¿åìÏ¡"c¿ÞB(.rý¿îõõO¢Õ'¿ï#'ŸÐ€UNASNone?ÄYþIJv?µ²Ì_z›?¨bÓ¾²?¡ÇpZ<Åâ?éh:MRèB?¸ÇتâC\?Ð	¯FÓX–?ÁÀ(]¿»?µÌ~§*žµ?³RÄå¯ç?åA˜‡°ÿÞ?ÂS\ø+r?â¿N»¢¡?°=ÀEà"?¾êé#r:´? ŸF"X×?Òƨ?Þ/7?ª¢Qe¸?à'k¢¿6Å?¦«ÄcUe½?¿ï5:ÀŒ?£N"r"½Q?×ìí2âT?§j&ôP?é4FGL J1209.2-7635?Ù:Vn‡Ù9À+×ÆÚD""À:Ûe¿wy´À<1"óg°@5°!›[;@›Y<²7ö?˚¸Å-ò?­&û#9t?㑺ýíV/@C%<û^?ì³vð!e«¿ÂdŽŠqÞj¿à&}­ªÈ–¿äÜ`ô6ž"¿×€´ÿÄ¿ïθʷH×UNASNone?ëY£$B¸1?²ì\T…f?|v["vD?sC›'ò4?ÁµÀ'Ô£Š?²{çl&¹ž?î¾4;o–?¥â¿>fí?aDԔ–£?nu Ä—?£
rÿ¦r?¥i°{kYÆ?ì$ˆ£S+? /%¸}ß?'¥äf&O?€ÕÚ]ãôÂ?ºp*±[Þ×?œ´ËÈ×6ß?ëå||•ªŸ?™åú©>ª8?À‰¦¯ ?pˆrCÜ
?¾Ø€ç±/?™Lðš»C4FGL J1209.4-6421c¿ïù™ƒ–šX¿ý"€Û\²ˆÀ9"$¼wêóÀ:÷bLLà@ÏrÅz%@#_=}9?ѱœÃ,?Æì¿o?ÿˆÑ•‰i¡?þ\3!•{þ¿ïJAl±Ú?ïõºAYç}¿äÔ6þÄÁ'¿ëôÿñ½G¿éÁ2?B`"¿Ùúc
UNASNone8?À'ájç?·1¢Oö©?žØ!¦£åÚ?Ÿ"è3†Š?ê膭F?ºÖÒIA¥Ô?¿k43¶"?¶ý-Êεa?¤Ž%?xw?¨msÝÊ3?êÉ·%'¯6?º®·Ú #Ë?ǪØhQm?¤Ý
9ýŸ?»£é{R?œ'Îq[€ù?æÃôŒÅ;?¨ÕVdäP±?Á¦YóãÉ*? Ñ'"ïʽ?²
âFÓ? @•æsæ?éTfAJÄÛ?§?/Rõ"4FGL J1210.1+3241¿ì³ç^ڒ@SÞ\å´$_À;ÅÚ(ÕâÀ<é(kYn@!\tWë¤S?ûYê¦Òg?Ù>4ƒ•KV?¯ô¾®Q¶?Þý-<ÏN?ýíôOG»Ö¿ïþh›Œ¹?ïúµÞs¾>¿â¿Àʶ¿ïsøö ƒ?î0?)á{¿ïÿ¸GʐUNASNone?ï¡ÿ^ú1?ôG×Ãs?(ì3O>ð?6ñ"|ëUá?‡w¯x?Ö+õ"j?ïhŸÕnÅ?¥îw`< ?hûH"'²¯?‡ìŽ¢S£?š3ƒÑ!?¢…HPhrÁ?í*¸ôØ?™öUi-]|?‡Z7X÷°?'-ðÛÑã¢?³ÄM:MV?˜?³°DºÌ?î›S¼ðêˆ?›"ìîÅ›?@ÒDõ Ù-?PîÖs'ý‹?¦{Ô?›ˆO)03´4FGL J1210.4-6250¿ïv·FJ3¢¿ÕmÒÁXzjÀ9XsHÍÀ:še"¯O@¦—Ìdòô@ø¶zzða?Ð"Ág	?ëøìæGÈ@s@ªÀ3?ùU®ˆ>(¿ê w~瑟?¼ÚÇ·9<¸¿ÜK¹ý<VH¿îz̺XV¿àŸÑß[E¿ïÿ2Ȫ(UNASNone?µNüÆ?³¬,¤Îó?ƹ‡œ·ÉO?À¯3JË?ç¡´9Qôì?ÆJ(dClÛ?™iøïÚMÜ? ®õPM2?ÇFÙåç?Ä0§¾u?ébùñ¡4?Ã¥Êi)ÙT?º{d·ô X?Ÿ$pžÛA"?ÏôŒ±qÿð?¯£Þ,°õ"?ä³p<¤ûù?±XZŽâWˆ?e;öy2m«?T"lÏcLÏ?Öù)dÆ?À¸mc4?än/|›/?À†_à‰yû4FGL J1210.4-6100c¿ì™Ïª«Bl?÷|…Ý$2åÀ:@ù¬(èWÀ;igI»4õ@ H.}ÁÌ¿@‡åÝ?
Ø?˪µJÐë?²ór}öÑ?íá8ÿûÎB@VÃÉBÿ"¿ëü'§:?ác¢1пÚ*{žÜÏy¿å¬vJßø#¿èÁ‹ ²'¿åWÃ Ô ~UNASNone8?É`é–¿D?¹…ÑÁ‰0	?'ýêî8ï)?£XՄ÷͗?éÖCˆ¶?»'á{:a,?Øw|¦Þ•E?ÊœàK…Ù?Œù¥i™Z‰? œ¦e{?ãP[êOô?ɤ'—žÚÞ?݈|ÞôJ?´²*/ue?©
DèÙ?"F<«\?ßU/:ƒûº?³Aå<÷*?ày¡|"¦
?¯Q"1Åx"?‹¬ä u?}'T·¢²Š?Þ4‡ŸÖŽé?¯f'äñ^û4FGL J1210.7-6005c¿êÆfäx@	1*À:n+ë†ÌÀ;k*þ±K@ 	ÃÑ%¡û@të<#œ½?Õ[H{úù?ÆLCe'Š?÷&q3I¨@$lÆÒ¸¿ïøcß"Í?ïÿvmD¦ù¿çQÁÚM¿æÂ:½k/ú¿áFmlêäæ¿çp$ sRˆUNASNone8?â¡XõJ0—?ÃU›%¿{N?©V4²'æ ?¤Az$ór?ג‡B?Ã!&»v<?Ô»¤á	O?È?{Ñf-ý?¬=aD4…?¹‹@	¼£?ãÞT{8?Èl#}ô™°?ÛY*Ì(÷ð?°¼ër–Ú?²d½[žÝ?™™
'l`?àÒîŠp-?®'1¨?Û-?ÛçÙd¹¯?²¡°eÁÂ?" ýæ$±?‹7΢Ï?ágM³÷?³*Ø'Ü4FGL J1213.1-5957¿î•@…šøÙ@ø¨ó©°À:Ç"hà"À;²þ¾·`T@Wÿ¡`bk@ށËFºÏ?Հ"ûOA1?ãÇkcü(Û@F{åS¬?üü‰Ñ$ H¿ï÷fÁ1
?ïúõ—k¿á£8I©"¿ä\«!Vfê¿ïþæŜVã¿ßëXZ4)UNASNone?ȉŠt@¦¢?¼IÚ
EÙ?ݐâ2½u?Ȼѭò?Ö*XŬï9?ř'‰ê§?¶»wL±?¹ž÷Þê­?ÖÖ4!ÜYô?Ëü'¸ö
?á½w{¯ä?˨œ1ÆH?Í¿Æ[D=ü?¨,$qD?ÓÜéВ«»?±q}NÁí?ÝC3Ë5F?°—©<ð¾Ò?·/ªàóâÙ?–ˆeÒ-s??×;r×£Ë!?´'u·—B·?á|Q8ž?³úã'ü$ö4FGL J1213.9-4416?ê·¿T>E¶@2b€'،À9ÿ'xë¤(À;÷%=§*|@c®%AÙ@[¹™ê!q?¼b?PÍÎ?ÍhŽŸ? Õ@m.¼«íY@aBŽ?ï»|þX`?ğÚ{aU¿åZ³uòW¿ãû}å3 ¿ëmª]6;ü¿îlЮÝ*UNASNone3FGL J1213.9-4412?Ã.GÛYJ?µ±1öX?æʔûâ°{?Áv7螣§?Á§d5ó…?¶jœ*í;M?ÑҌC! +?ÅB»ÙÎJ?á"Éà>|Z?Ê"+"ì'?ÆG¿øÂÎA?¼¨®1–??ÝLk8ïrd?³íÂu?ҋÉϽ7?²8ñ•"?Ð("ý@Ðe?©5ssÒÑ9?Òlvõ\?¦æÖ2–[?܉çȄ¤ ?°ÈtoP¥Ô?ÑZ¬3fƒ?¦6¥;Õ.º4FGL J1214.5-2318¿ï·Žì0Y(@Cc‰!S7À:ӕÄ"`À<o]2K­@\Ž´
c@?ýהÁÄO?Ô(ªÄbC?Ñ.…dˆñ?ÿÏ'T·@øSK+¢p¿ÕC	ËÜ?ê#X)ŒÁD¿Ó¬¡«¶Ó¿ÞӎóMj¿äøSδ-š¿ïÿ7¸Óñ"UNASNone3FGL J1214.4-2315?ﲈîZ-f?zñîª@W^?S×hká?O¡…"?€â×\ªI?yí—æî«?ïqª˜Q?Æ2ýÞ¾—?Tç"iœ?c/³¬Xå?Š@|•Û?‹©aY'?î0%yõ4¢?­=­Ç3¨?ƒ'•{ñX?w"p°ú¿A?¨6C»M¹–?ŒST˜Ý"?î%㋞ÄL?Œ
Io¿?vޔÈÅ®Ò?eÑã&ào"?ªÅô¬ûj?ŠüýÞxõG4FGL J1214.7-5858¿ï
Š¯Æו@'Ä$#À9¦`;©ú:À;kT/,=v@ÛÌ{O,@-¦¿
"?ÈïcЉð¯?ÁÏ+KÞ$ä?þ<xVRòì@•€ZXf?ËM¹Ü°¹¿½håq´MO¿é^´ás¢å¿æ1neZοïÿs³VB?ï¾h…ûW$UNASNone?ۛV¹œ-ì?Â,­¬×§f?¢ :cŸP}?ŸÐڟ?áPü÷ô?ÂÏúŠÓHÌ?ÖВZ¨6?Êê0(FÓh?¹geã
?»	²ã®?ájÔ%?Ë6$eáb-?Öd2;@?¯bH}êÇc?¶#•'9ë"?•Òä'+º?â	tL"…?®Õ]ÙD±X?ØWtû(]?±ö<À'š=?¶Q>Ù?Ÿ•3ébÿ?áÛZ©ö]?²4œï[Ä´4FGL J1216.2+0537¿ìeC'­Å@P»>-b9À;}JØkf€À<¶]ŠÒS@ R"²,?ÿ«cÆxö?ÕV¶JªH?Σ€ùÊ?êžwïû¥þ@	&'=TŸ??¯®Ï¶·Å?¨Ã=ë¨¿ÔÝç®Ðc¿åÕuþ3÷ÿ¿Ü4ÄØ·'¿ìÐ=ÊeêUNASNone?îÚtðWH?§58SÜ
?iutg*ö?göÝÖýٝ? Çé£HHÝ?¦OU»‡oŠ?ï@áî?˜J>Û4èW?[ou–vÀ{?pr…¿G"?–,æ(×°¾?–)ÈéSj?í¥@;úý?š[äl¼?"ëM2µ©?xî%"ëu?°8"ƒ‰Ñb?˜á·ë§t?!β?Ž"¨¶|T¤?b«g¤¿,ã?X¦—PÓJ±?¦
G"—"?ŽœI,&4FGL J1216.2-0600¿ËÈ-ß>òã@Kå2µ^ñþÀ9ÈÏuôxãÀ<,νgÔû@¸™nÑnó@—¯ê=öÜ?¸óÓÌÆAÃ?½Té;mie?þ±Á
{é…@D,²™Æ¿àsûz_B¿âž.>VÒ˿蟦=ìʙ¿âtŒ>'6ú¿ï¿¸Så¿ðUNASNone3FGL J1216.6-0557?î5ŽÛž1? 'ª¢'ˆ?žÙð2Wœi?—1¡Œ=Oƒ?ž¿]ò4p?'Þ¤'Þ?ì
334Õ?»ØdroW?¦3*Ixp?²sMž²©¸?´"Ñéª!Z?®e±ó>?ë·=»?£ê~È
6?¬ænH} ?™‰™""¶R?¹o
3V?šœ'Ú˜ôè?骶O~h?¨b"yÈðf?¾ÆŽ¦°?¥Ž#m;«¤?³äJôf?•q}àÃ×Q4FGL J1216.2-1550¿²TBô«7@G5ü;OaÀ;W%­AíÀ<šÖvš@ JB¾@
¤‡3f?Оi¢…üY?®®£Áæ"Ê?߸©)Y•ž?÷¼"*F¦?æáJ2S9¿ÕãvÇÝyÿԒ/BêÊ¿çÚ\FQô?—˜×…k¿ïðÃhŸýUNASNone?î*Fž9\?¤vá=»#?fmjÑÉ'?jó¶oJ\Ê?«ôÉ(ÿ×Ï?¤'méÍ?î6h+0a0?§¼Ù?ž+ž?wRð*D+?"­L@ÉÜ?©¯G±g¢?¥sbÖ.®…?íW¸i_b?–`.#ò¡?ˆâô"\&d?}KJ†ÌÜ?²%àÚI€%?"à'¼x)Ø?ë ÿ—¯?¥ƒ{_놶?|gâèك?w°h"ʱ?ÂäCr‰ý+?¥Fݔ"þ4FGL J1216.4-1358?ÚHqL¸.I@HŸU›=À;&:Wê£À<…AøDJ@ [&¤«@5ºÚ\‰?Å}®ˆ*Ü¿|8ù" Ðý?¶POx¹$N@<€;¤›Ö¿ï·1Å?ï îؐO?ÎH»…§ŸA¿çviéпïø£NNB?ï인KhUNASNone?ï°B£ßP?ƒù¤ätMº?R5êlÙC#?S;ν©Ëc?¨½Ém¥?'òH%ðDi?ïru«{:?•[5ã?P«¼®?cm=âr?½–'"ͽ?"<µJbÎ?í;W4NŠw?›.'û/Tc?"¤YÁî?Œ-YšÂÎ?°üBWµ;Ë?–‡	?Œ$…?ïAaRœ?".47+i?iS{֜SÔ?g.û«ZÉ?"³y"?'ª¹fHDµ4FGL J1216.8-5955¿ïžB®®Ý+@>ØÓkLÀ9bsýþžÀ;%‡\€3—@/ÛåÄj@¾S<½öp?À愙WT{?Ï{£ºY؎@9[Ývh<@èÀr×
?áRá"öW¿áôÁÞ\A¿è9Xç!â©¿æZÙ㐿îgñ`ªåœ¿ïåaHÌ"UNASNone?¹ÞMÐÅJº?­ÅÊ †U‡?Ü$Îÿ˜Ï?ÃÈâbýïb?ÝcŒ6¦ƒ?Ä\kßoz"?¶#ì}?
Ó?³Õ¾œ­x¤?ÑêMUdÆ?Æ­å0ªª?äF[Å¥»—?Ç\
>OQl?Î&á;î"[?«$Û܅Xÿ?ȱÄ-€³?§SúåÛJÛ?âIÖ¯xþ¼?®YS£­?¨)	Ý)?ˆ:?'¹‡R?Я¶Ì–E`?­6^{jño?æ%'¹#~?¬âå|S[4FGL J1217.2-2500¿àQÖs-ò@B›ÿñÀ;k$á`؈À<Ô¯«SÖA@¶E‰÷æ@>¢'vge?ØfÜ­ë`6?æ—r½·±@
›©ÄŠ,?üüøÔg Î¿èPä>X€J¿á Îï¼¼¿›à®^«9³¿ãêv–_Rv¿ïÿà•V"¿ïÁa)ÃÂUNASNone?ävœz=…?ÂDêµ-¥?ȉ´'†ø?ºŒIˆ-±?Åxpûå?»µØ»ÈÚ?ã)åª<(æ?ËTzmü?Ï¢ê<¬û?Ê% …õ?õbaT?µ*6@øõí?åOð¤7®÷?¯ÝyW²?ã^*rC)?¦XgO‰±"?ÇßD¯þ?¥IF/J:?Þj-[Fü?³÷¡¯Jõ?ÎptÍKo?³Äݵ?Ò]Àƒ¾M?±¯¶I¿÷t4FGL J1218.6-1049?á°òA.&7@Iœ,ÂãÀ:´'QžXÀ<L#{/KG@ؓ…ƒb @ßoijù—?Ӑ¡7óŒT?á6,­4¨@ó÷ ]m™@áÞõnW?ïÿ·hª¿Û'{°)©¿éhÚ´ìÜ7¿ð?ïú—á2µ_?ïÿ¢bôUNASNone?ïqÎ֜¾?¤|ù^)?n6ƒ©yPw?…:•S")?Œ{_ú|3?¡Òþ‰·¬?ín¯Q-pº?¼[Œ Éì¤?™…~èå1õ?±lmg"ªm?¬RKx¶[f?°ˆš¥º5Ö?ë'Ügzà(?¡´&pçɉ?¤f¤ù
`?ê7'N®h?¼Žq¬yŽ?œßtè%J?ïo;/00?'±ÄàÒñ?Hðû3:?]ñNÁ¤Š–?'Q@aYì?'Ãxèݵ4FGL J1220.1-5558¿ïåFM8ºS@ŠŒ›"UeÀ9é'Dé>À;î(«ð´3@ßG`'»)@µ'-lJ?Ã+þ +ïr?ţܾ‡d¹@Á\ºT$@tÔHD:?調.%­¿äëEÉ7ìÖ¿àÒÿ¡‹U‰¿å(‹¤äPw¿ï±‡¿g¿ïýyb—yÚUNASNone?êAº;¡%1?»Pe)?ÅÉ?ÝMh£?™¼k*á?Ã=sGÎVÛ?¸ãÝWP¨I?Ýa =eŠú?ÈPmM2Ú?¤aäÔuàF?ªMÚ¡\q?à	Q"Ü~?Ç:XušÝ?é³¼—ä?«©[,:.?¨AšK.I?"]$žÝæì?ÅèÊiÄÝ?¦óªV?37?åªóßcœ?§,]Øv?±»Ê"¡Ù?–rÆpC[?Ð;%¾àQ?¤Ôyam4FGL J1220.1-2458?ÑdêüÉÐÕ@B­³Ð|"¶À:œ€šÅÀ<c«Ø`~Æ@ _ºª@TXÍ ¯£?ÀmÓÃ-¿‡<3•ŒL]?Ȭ| 9›Ø@Iۂr6?ë|¿€^	¿ä)ôÆ)¿â<½ ‰ø½¿ÜB_ !¿á¡–
W¿ÕM!ñÂO›UNASNone3FGL J1220.0-2502?ï3µ×´?Ž ÷rôÀf?p}ªh:y.?c
€U=.?›ªúß/?‹¾ˆµ÷Kÿ?ïQÏކXs?Žó=ÿ?QG–×öÛ?Y–FK¶?"±ŠÎçr"?ŒìAm<?íöiˆ??'
ÉÔ½?w¬P ,Ô/?a*'Eò±Å?­£å*Áá?Êçô~0x?íigÛS?̶€f'?ƒK_Åë?kÓã®e+S?²KeÓpgõ?cDñû4FGL J1220.5-2745?èûYuš¿g@AMçê_"ËÀ:zÉۀĶÀ<>ðd‰Ø@wQ-=¿@¨tBÇû­?ĕeTB¢?¶Ñb?ïf þ'@Iòµ>»¨¿é­ûPm׿Þ†nCªz¿ìbÁì!¿Û"fy±œÆ¿ìÿ»Ëǔ¿ïÿ\l¡UNASNone?Ë6#?žÚ«Vêïu?~Ü6%?Š˜LŒI?Ì « µ?—5ø'À#Z?ïJi'ásh?">
Mp?bÑøDÙ?r"1âà?"p³dÈ÷Û?¡‹j?ìþPò
ý?š°ƒ*ú¾œ?"Xç‰Ì«?…¡çÉDr?²ù$~4ê?•K»Ÿ1ç?î‰kur.?ŠqÈow5?Ž7E"ï?{bI4ÑAÖ?Ÿ¶îÆïÈq?"ŽtA€Bù4FGL J1224.6+7011?êõD'@GaFÜ]cˆÀ:\H»Z´À<PÑæAq@ ­'ÐÅ@7ºœH ƒ?¹Ð­'ÐÅ¿¡ÊžÕ˜£?ââuuÍâw@]/ÆO?ïÿ
¢q›¿æFIlÊ.¿ë ²Ý¸Wu¿å¸
ñâ¿ã8?!(οïÿøþÙå9UNASNone?ïØ~¬? CØìp@?plÿì+–j? 7–BÞe?L—Þ¦˜œ(?L¹•ò?ï@q;a‰?"·¹Úá
?]ŒÉ\ÖD?jòÞþž¼J?–þa–?'ù>Α	=?í¶
ÆÀˆ?"»A#y?†µCxóK?wdÑñ9ç?®ñÒӟêª?'b"w4<°?îõxiªž9?†€@æ‹ué?¯àŽáy"?Sz?'yƒ;|?xþý"ûê°4FGL J1225.9+2951¿ïê/Ÿ¼¸@Tñw[0À9'7 þ}IÀ<@̺XV@±È,)(Ã?üT¤MQÂ?·JRŸ	E#?Ú÷FóÚWÐ@"Ðàm"@±a5$$"?ï•¿,{3?ÌïÒ Ì=Ü¿ÑPLH­î»¿ÝΌ 6즿í]¨QÃA¿ïêo_‰RzUNASNone3FGL J1225.9+2953?•ø>?tè?•§Dá°/?îô¤ŸþüÅ?nVMâ4K?†æ[Vþ¾?‰{ðåùö_?²–ý€;ç?Â5ª×^?ì*É¡sý?ÅÐ4K:?¨%j误Z?®QXtì§\?¢ZwìÚ?•öÿ=æn?ìn(¼#5R? ßZµ?³a~(¦?–(ôl[ÌI?•ÏÚ[êi?…Q›
Ñ?ì7nyܛJ?©íï…d?¸Ð•šS«?¥¤Ë_Dv†4FGL J1226.5+3023¿•ªÄuv‹@TéªÍžƒäÀ;A§
›duÀ<x
c0Q@S͍'ùg@ÁòÜ+¢?Ì¡›†-Öþ?™]g—Çe?È01¡Õ{@#r ÜY¿ë^¿¨÷Ûn¿ÙhòÝ­š­¿Ø@ãȑտëÞ
Â5o#? æPž`~¿ïÿ›¡[¯ÔUNASNone?í¡o#:mJ?¶"‹l]?jÌ>=b©ê?g9"'?²$ôA€]?µýÕ¨ø?ï(T‡[é?£H€OExK?[¶¸š–ðç?sì£rÝ(™?™:ÅkÃ?¢gm%÷€?í
¯Ý΁?™ëÛöæ?6ø_[+?'Ê:Ú
6S?´¢
 ?–<[Î;²"?î;›Qè??—™âÃçð(?`NZ{àýH?_s,v†ûŒ?­ç`£#l+?—uÎÁ團4FGL J1226.8-4907¿î}+¾ŽŠ@+ÄÞÁÁ×À9}ÎéöÀ;PÜ¢b–@	ÛhQx@B Ž€a?¾ß¡:ͱ?Ç=ýçvò%@H™|=h@@
EBÉ(R…¿íóû¶Å?ÎâüúgØ¿êO"J'°¿î«ØáX&¿ïú	.Îõ?ïá c¸6=UNASNone?ïÏ«þÍ{"?›8ó›P?UéøÜ\:?ƒÌ#	ˆÌq?r¯'b=?'¯C·æn?íÏî÷µDE?µ#÷xŠ9v?']'Ÿó¾?¦'!)	ºy?ªRG4²2Ó?­z±gcQ2?éÿæ
TN?©qmx±pu?©÷ž%¿–¨?—'vá
3?Á'€A@
?¤µJ†&?ë²Ì´ÌªÉ?­Áˆ	~1?ˆæ‰"öa?{Â66a?¿LÉ&ûݘ?­]ó1¿Ùd4FGL J1228.0-6918?ç¢H(ÛÛÀ#âOëОÀ:ÇM~8DÀ<)©HcF @Ùe4%m@o«Ú
ýð?ËT3]û]Ú?»(‰Œ\`?ð•¢y<,?ý9+€À…?íKT'
`ç¿èÿ §?tŠ¿ä|<& ûù¿ã.÷ϯÖ¿ç…ý_çœ1¿ïŸ€-·É0UNASNone?Ý¢¢TR°?ÀõfEÏK?}›ÈW½âÓ?vDÚ°"®R?àówc&Zá?ÀöJ[ےµ?Ú/6ÂP?ÅaA¥Ðُ?x¤9ðš?ƒÀHh•?â·‡½¼¤?ÅfŽSãöo?èM¡Ã¾®f?¦O]â»í•?–áôýÉøÕ?~PT½)Ì´?Ëí:QLJ?¤¹Tx"|Ë?ç' –?¤Q~¾pÕ?üTp©™Û?…VYŽá¡?ϣ󰌶?¤	¢'&½4FGL J1229.5-3048¿ßzÅ	A0@?Ó ù	kºÀ:óD{ZrÀ<e†Üþs@âƌì¸@»œ"á?ÖØ­Áä}?ÉäbÈ!?õH(¨•µß?ú`ŒzLL_¿Þ)Q¨,Y¿êR½<6¿Ûœ²þšz?¿çEa-¡¿î	‡"s\¿ïêvUNASNone?ã*¬QZ+?NjóþQK?–ö(‡Üö?¹(ä=Bd?ØH÷û^ÍÜ?É}†9/¬?íC0Ë÷Ø ?­V/¢ÜåQ?'äO?¾?"^ÒÙ¶"ò?±ÂŒ|+?§_,lÅ©k?ëÃ_¢¦"?£®ÞM
[¸?§ùЇ«–r?"'#*$C:?»Ìü¿ª?'M5Q¿…?é_€š?¨z"¬»Â:?—˜¤î¸?‹Ž¸\UØ?È¿oeÝ÷Å?§™kotù4FGL J1231.6-5116¿Ïe¼ðX:@&÷\òI^À9ZZ¦>ÊÀ<z>ŠJ@F:ωÀ‰@fû_‡O?¸4€·å#?æj'ào–ç@'•€^_0è@¾€JGÖ?ïÈÜ}Cø}¿½Þ½åÿ"à¿äw݇/3Ê¿ïi'2t¿ð?ðUNASNone3FGL J1231.6-5113?»üOî›."?À‡œcò½ß?è#uŽÌ®*?Ì/jç·co?ÁtÍ°?ÂOi*x¦?šàíäË9\?²©F%Ù-Ä?ìÄÖÏѼ?Âü>U¦·K?³!€N£Í?¾¨ÚÅêÞ?½EË\ØÅ?¦""{B?æu14±?±=ÄTg)³?LjUí++×?¨NÀTòÎ?sü|ld?hcE¹ÏL×?틞H%Í6?£$ @ÔÝ,?²cMg
Ôw?¢>X½Olï4FGL J1231.6-6511?çÀ­Ù©TÀ6Ÿ~µè…À96‰@†
À;9åèý"û@ٝÃõ¸©@"dEú¶?Ân D2Ò?ÝÊBÄJÈ%@ɝ_÷·\?ÿ'—¿ïÿÿ)@k*?ïÿþˆ0»Š¿à¿"àT¾ô¿êŒ@À}¿ìý¢yM¿ïûîיåUNASNone3FGL J1231.7-6513?¤ß>j‹+?³%†
°Ÿ?ÛuD²K4‹?ʜ¨|¦š?à÷i¾½?Ë
'¢`,7?¢çÙnˆ!?¨䎄Â?â;T¨ÕË?Ë´q¡4ɸ?Ù,d"Òƒg?Êцfõy?«R@Y¬_?'ÿ›|•$ó?ä†l.^?³÷(ÀÊÆ=?ӈߘ
]s?²
¿aD·¶?®¸ï.'ºn?VeR©M•?ÝršUÓ®?º£Ö6†?Þ¶ÕÙÕ?»
e'>4FGL J1231.7-6653?ꈛ¥7‡ÀcËďªÀ9ðh¬'ÃâÀ;G¸ü5p$@ÕúK`%°@¥EŸF'?Ô͍Ý"ÛL?ãÂÜSRl@	ôŽ:!d@!$‰w7š?ÚþcGοågÔôó¿ì®Êžc˜¿ëiäñÒÁ¿ð?ïþ× ¿UNASNone?ä!"N_?Æ7œ&ãÎ?¶¶˜PÃ?´6Àpëƒ?ÑB1O?Ä
GëÇ?ѯœy¡·‡?ÊËïN·?µÿo5Àڂ?ºUØ]õvø?ähCÜwî?Ìi†¼M˜?ÖÍ4Švÿ?±#3;·ô?Á`›—°{É?¢EÈ1n?àAJÿÎ¥Ž?±bÕº¤Ì?З;l›–)?²§ø'YÉ<?ÉEž¾0ÓX?±ö·€.£z?ábúš&?¶"F;èœ24FGL J1232.1+5953¿ÄMÐ*ØÏB@L‰ÄڐïÀ;½—¥¤À<³Ùý7@õH&4r#@	=·ä{õ?ÊÈü]´¿®RºÀŽX¦?ÜüϞä1B@v=}dá¿ð?ð¿í9~¦Ï¿ïÄ_@¿ï0_y[X?ïGâ¢w
ÓUNASNone?ïÜl[ à×?'w®64ý?^)7mû—ÿ?nó§¿HtM?d¨!],?ùaC†#?îݙÂ!ŠF?§rrå¬Ã'?u¦íL\?'å=Î7?žãhÎ3¬?¢‰Ž¹©¹?ì)ÄôÏ? …x_­Ü?—¸'ýÑêu?Š—NÔ׏ö?¹(§à[Þí?£ûéfß0?勒²<žþ?|â\:X?{X:-YÄÝ?xÉÜtµA?qÞl´V¼?eó¶'ý4FGL J1233.0+1333¿ÁVUÑ\˜K@RðÞÑ·À:ü˜lrðÀ<B½=ã^@&Ø,ý9&@§ …±…I?Ãd´ CŒ?Ìf7AŠ¹Ø@ä†&ö@Õîßq??ïóçÞ¡
§¿ÖŠîü!¤¿åß«Ì¢¢¿èH'_ì#տ뒥2.¿ïñ">¿UNASNone3FGL J1232.8+1332?ë0®÷ô˜X?¶]»UC½?œW8QŒ•7?"ܥƤZª?¿dº+øð?´ÿ¸KeA?íÙ—›ã?¯¤*W-x?'Ö9*Ds_?¡ªK5ǃÐ?©éñ,¨?¤'ëΙ÷©?쇠,³?¢8?²¤¿â? Ó(‹'?@œC+Ó?³·
ú^Õ?š«#ëÃ×$?êR¾
‡?¡Ø'»<́?¹¼úl2?ž4´¹ÛR?´LöÖÍ[4?"l¤÷7-4FGL J1239.7-3455?ȵìx04É@;âbS—À:ÐDñ¡˜lÀ<Bãü";@äÊ-
O9@%1"Éÿ?Àq2GOõ·¿³d$í ,?ñËý™ô2@Y±=¥'?Ò
»Då_¿æ¦F…öN¦¿ïÿô¬å¦¸?ïýŸêÁ¿Ñüê
î¿íIhÉíõ<UNASNone?îr3;ý+™?²à¯sY8?™ÄN·-üº?±Þnۀåž?—õIÉ,#?™z!†½¤©?ï¸cňí?Š,"™î?L.Î3u?y7ŽS'Ò?€$!ºÍ‹ø?ƒ?»]ó5û?íÚS‡N`?šƒ®Ra^?€ÍîË?r'üœã¤¶?´ÿ{‡Ë+?™"WP*"?ïÇqfZÒµ?|ñõ¦¶?WäSÙ¡~W?p‡!ëþý?vN7Ü.F?wK\"r?4FGL J1243.5+5311?ïûОœ}@Oñ\(öÀ;´vTðóÀ=C'üÇf@ cõpÚވ?þ*(,nô?ÔªL¤ô@¯?±Ž%È¥j?ÞzÊáæ'@x8֋<Š¿ë$ñ`®—¿ì.û€"dü¿µ™ÆÿÈ"¿Ô*¡OÆ¿ïx×ì;?ìÄs'-Â0UNASNone?ï…6ÊĈ?',ëö…Í?C4tó{'°?E®B¾š
?ÿ¤Ò?'ô«RT?ïPªæ. ?š8ᨮ>?SÀQ>h"?ip´0™žÄ?"®ž*"ºà?˜Ÿg»û"?íNíˆá^?Ö
mó?Ž¶—ZßÑ?‡Féë~¸¡?³fµ°-™?šdœòþ¥0?ïœR$›\?v‡É	RØu?Káé¦êž?IÇÓ~̤:?‡:øß>ºy?uÝ%G~E;4FGL J1243.7+1727¿ïèjÃJö|@T
¯%;À;9@À<Ù$H¸@ ‡Z$ää@\ú&¢+9?Å´ØÏå[¿¶9÷GŸ¦Ï?壼gú»?ù"€€Ce¿çGìþ›{ò¿ìDåýö:"¿Þ5'm,S¿Ø쮿p˜Ä¿×`^l¢¿åIÛ¶t›³UNASNone?ìͧ…õ0?ÅõeJ­ãÇ?kÉ7[ïÉ?|:Ny'=?¸µÕ­vý?Å°
L7(?îƒ/½Z͸?ª"ÎçãØþ?rÑ4ӜÒ?…z54­º?¥rݏߢ'?¨šíö\·e?íaYìDÒ?—Ÿ‹f¦?{ë.þ¹{?pü×9›é?³6}­ø¤W?•øBý$ð¨?ëíø
"«?¥TM(îÆ?ŒSˆ>r?"%eˆ<s?½Æ«bÝ?¥JÜ Èr¾4FGL J1244.3-6233?ëÉó˜Wi?Ӝ?{Àë˜À8Y®4[Q_À:Žž @7Û@&ªfpwa?¶Ž±3>F?º×Eâz@ÉÉã
€ò?ø8DD}ˆl?ïÓ5!	†¿ÆgÆ£=q¿ãg]Ý*é¿æÞíášdE¿ë›@˜vƒë¿ï.
ß¼"šUNASNone3FGL J1244.2-6227?¼ÑÑúC?®-5ÛäU'?À³3§û	?¸Ýÿf?è8øó!õ\?¾ë2
.¥Û?™ÃÌMálh?Ð¡Áº½h?Ï`|ë¨?Æ6[—+a†?çYß¾Š¹³?Æ%>€¾q¡?ÁnŸˆ85?¢÷éPR1?Çà€ôós?©€ˆ¸±®?å¬7ü\u?­Ç~‰+?ŸA+\½{?ƒõV<â¨?Óáª^1Q¿?°ýiø!¾t?å"—Œq4?°õ¦²˜4FGL J1250.8-5424?Ó«³fþ@ î)Ø@žVÀ:ƒø³o.À<Ï<é•Z@¶Nií"@qº?À~ÀzY
?"0'—|<?хX.•>Á@•x´Ðì?ïÿdd-§¿ÖЏ$Äì¿æ8õ³¿Ù¾@Bo	¿éŽÌܽ¿ØˆUg"UNASNone?áÛÅkî!~?Á²ŸytJY?"P'&B¡Í?ˆWŽšßÿ?Ûl¿'ç?ÁŽŸ²Áç?â÷œ¢¨uL?ŪkóFÛ?v_
»Ïå?ƒ±iÇü)?Ù·JÂš(?ń¶2xêý?捖]|û1?«ý—pÙå?ŸòPUìù?†<™Uó?Ðå®?§:?©è›C•?ëÀx<e\?"ôÆàRA¯?Ž8|^Ê^?s¿ Å?¾5."s"V?"Øa"&—i4FGL J1250.9-4943?Ô"Îíʄ"@*M~Ë·ù×À9ñ¿³ß•ýÀ<8#;nk@'.íÿ"@ÿCB?½jtËáY?¾ÖÜG©ã@Å$aß@iˆZ?ë†+'Ëöä?ÚAžlK¿äÏ?mÔñ¿Ñô" áw¿åˆë–¼o‡¿ë:ÿ[ë8UNASNone3FGL J1251.0-4943?ï_è¸oUú?‡¨.ZR:?e­s,ŒŸœ?a'©-§Âx?'M:Œƒ¬Å?…âb·&Kj?ï0ÏåÜB?"áw±?eÚYQE?v±‰ÎnÇ;?™–*¸OD?›<PW…-‰?îÀ½¶±f?‹.dIVΡ?qƥő4R?dã€&ž?¡»OÜ<ÿ?‰ ٛ?íÊ:¼³g?Ž,‡êÏ¢?™aU?ùp?¶ò½š¸?¦«Î""Ì×?…®ï¸ŸE4FGL J1252.7-2520¿À~%¬¯Bp@B»ýq°GÀ:£9Œé‡îÀ;ëô9rè@"<͐Â@RoFøÍ?á¥ô@")›?ÕBTcY–Ÿ?ðèçÖyõ@…ë´½·¿©uy~Çc?áOmŽo¿èM_.cÀš¿ïqKÞ'ñ?ßÎùã0fz¿ïÿüÉï£UNASNone?îY±AŽ
?°8—DmrP?—`_ZÄ¡¬?¤u¯ƒ?ÌL?¢Š5>"ÎT?¥z¿ƒK?îÞ-4{½É?§¬®ò!åR?y‡$ܐÉ?"£[;L?Ø˜'Q"§? Ü²®Y2ƒ?çêEè'Ϻ?ª´Éx'ƒ?³`äO#Û·?œg<¤f€?Ʀv6&Ó9?¤TwC|¯?îêN¾v?•<G&ã»?5ËÒÃ6¿#?B7¶:J¸?¡/†®'1?•)¡¨P_E4FGL J1254.7-4516¿×G2¢R¥@1—Ö[åÚÀ;…Y#‡Ä…À=gû'@ RTN‹Ô4?÷%
`¬B?Ö¶N›™y
?鎥.i@g›\è8c@ʈˆ¥*œ?ïÿá'¢±¿íä‡imP?܄",tþ¿¿)¤i+g¸¿èý0½b ±¿ïÿýawUNASNone?ìy¦ž¬@Å?¹ºLS††?£1®æ×j?¢–5Ö"Êó?²™ó—2DÏ?´Ê:JUŠ?çò•"vü»?Åi#hï¥?·9xœNï?»t‰ÚÂÞ?ęõÕåœ?¾¼"²??éá'Þi€?©C%҆"?¯_³<'?šRû!x?À¢4ZãUš?£¦^½5š?æ;|×ñ	?±€ÑƂ…ò?¶AÚtþ$o?¨*\ÜÊ?Ëñe¼Ý¤?®¥€[î4FGL J1256.8+5329¿Æ©D÷Á@OÏÞ灃ùÀ:A'½µÕÀ<2ºOò†›@¸b4þdt@@'w?¿JriÿÎ?´Å–¶eW?ñ~@'7|n@Ï&ݺZÚ?î!၏·™¿åPʽþÓ°¿ép¿ñ7n¿ä–fr•I¿ïÿ+Žúg?ïæG\µã|UNASNone3FGL J1256.7+5328?îàé«[§?˜¿nøOµ?"ÊnÎç7?Ñg,ԓ?Ž0¹#Çô?c™ñÔ?ìø櫘Ó?²kz½£>w?˜Sæ¦yuÝ?¡b*¶ËÇ?²#Ðùœ³ò?«!tãúû>?ìw'-ÄX?œq†n~úé?œêÀ©?‹Sz·áx?µ;ôA²ý?•š¡Û?ëøÆÀŒÕ‹?¢Ý¦@=Cì?®®ÍúS×?›#µ«5È?°âbþo˽?•ÇJœrµ4FGL J1256.8-1333¿ï?A¹*P@H¥VHþÀ;-Þ5ªÜ¸À<ˆK¹ë@KsÙ@¤@}= t.?Çè£ØaÖ_¿¤—±U±?Üí7OË@ëFƏq¿Ø/›#1ˆ¿Ø‡Ø_ñ¿ëk!ÃI@¿ÄÔèå‡-Ü¿ál‹ä¥0§¿ïúlb~Ð@UNASNone?ïJ©kUý?"¢"š*?^cÕ'd?U[uÿa	?›qÅBÎo?"GFTËd?åµûB?‡®J§p1ñ?COeo·C?Qù¢çQ'?Œ¦;…¾?†²˜åðÝÔ?íä ö#ÓZ?"
¥ò³¯í?~ß쬧HÃ?m¯Š,'§Š?­Ùó-áI?'h1•×%Ù?î×,$׋?‡3·ƒ"úr?iQ܉t#?]BÅ0¦_â? ø÷KE?†Xè2|4FGL J1256.9+2736¿ØÓcK¶@V+©¨–hÀ;äa1sÀ<£u»mÿ¸@á#õ[â@Š;WÄã?Ѭþüôã?Àå—IZè?èi®ðBô@ïƝޢ¸¿àf» Õx¿Õo"'`í׿ì•C~Yø¿Ô[€–é;¿ïýîþOü˜¿ïóöúUNASNone?直_pw?"¿qÀU?p¿äùŸ'Í?qiÄþH•+?yëëN$à»?}Á¨¶@[X?ï]ëeÖv'?"Ǫ›cÔù?_9Ôv–O?qvklðió?'OÇéѶ?";±gíp†?ìüÃW}Šj?šÇkð¥‰?'啐 Ô?'±B€.?³ ß뫳?—Ìþߜ?ï;Ïgßø?'u"G¼r?ƒÒÝOÇ×?wvÿ?ÏCi?9`–ï:?y-wVÓÁ4FGL J1257.0-6339¿ØTbtá ¼¿éO0«¼²À9=Åté¶èÀ;nããiÇ@8¯ÿ;_@˜«B8‰´?†'vçh?՘" ;^Ñ@
à×ò›?ï,é™BS¿ïýð@o[Ø?ïÁW]ßÚ?¨f]O³¿¿ä-Þ)ìb"¿ê.^¸; ¿îD$QîàUNASNone3FGL J1257.0-6338?«¸>qo¦…?©ß5à¹?´_wEÀÎö?²t†Àm¡?븍00ë¸?¹" ­,Ÿ?¢Z¥á1¶?¥EîÃð<`?̇[ÍÝy?Ɓ¥Æ™u?ç¸~®x>¢?Æ]"=Ö'?¿y](0z?Ê²ÈAs?È®5œ…n…?§äÁÍ,?ååFóÞP?ª]¦i–‰»?¬Q-®4ð?"øû/K¹g?Ð16œŠñ?½ #ãE®J?æ'Ÿ$×9?À ŸÅ¨²4FGL J1258.4+6554¿çÄÌQ
	@IšÏ¿ÆT
À;"åV0Ž=À=%|'K@\P¡X)ã@¾Àdß}©?ÌÍ¢à•+¡?'wÿ&L?Ò%œq».@Æ-Ní¤¿ê˜›î¿âQ–?òß0¿îÛK_ú¼t?çGÍ+¿ìÚǗæd¿ïÿå"m/®UNASNone?î'ü¢³w?±@z Lü?‰2,j/P?®¿‹Jco?žûғjY?žÞÑ5¿¯š?ï ¦uô?5QîÏÞ?Kð
­IÒ?tºP×_@C?†:U‡ç&?‹ÏË!€û?íuÀ²Ëm?›É –ŽãQ?‡+¥¨vº?~2ñã·ð£?´ÞÝEh•»?™ãcðÅ
?ïěÚSw?s_¼%áQ?aÝOö¿!=?gØڍߢ?tÃkv³"?lŽE‡¯ú4FGL J1258.5-3406¿ïÅúÜ»¾n@<¾š,fXÀ:¥{ 1ίÀ<U /Äê@Æs—Qj×@@D
û?ÅÆ÷ܔ@?£uÌàÃÏ£?Ü0«½@>älP¶¿çž¬ÞšÕ"¿ã¯=šÀ5¿å>#¶e¿Ûa®[G¤Y¿ïúûHáb?ïNž=î"2UNASNone?ï
eãõ
I?•ÔÄÚÉ}b?m1|p?f¸»>ŒXÔ?š­ð´w?"A!ˆ?îý†[£¢…?™†'->N?f!¤vW?s¾|¹cSø?ŠÿüËDR?–Å{Ì?í^oÂ2b?–Ö} E@®?‰Ã<Nô?y{L™¸}?±Ü‰ŒŽã?"Ä6·Ûl?îFò]‹ˆ?'VÇ+ÔD?v_(Î
¬?hfàtXi?¨Äõ
†–É?'XJ2øÎ4FGL J1259.0-8148¿«ò$üâßÌÀ2òã'÷ÓÀ:4·b|ØÀ;úÏ®ÿ\l@U-ß6[Ý@1Ze§#Æ?ÄETÈÚ#ø?Ö ÛâêE"@:¤vlmç?ù­q:)òm?ÌÆQ)³¿à*_"ÊÕ|¿ãnO3Cú+¿é°¥ŸaY·¿ïýá!˜¿ímî$nUNASNone3FGL J1259.3-8151?Ìr¶ÖN‰ƒ?º­ºe›í?ÑÐËÅ{'?ÂËP0d$?ßö'É?¬?Ãá}֟àü?Þ°1´»4>?Íö|¤Þ?Ö ‹¤"Õ?ÌöO¬|T?Å^…McÖ?ºa]uޚg?Ó+˜~G·Û?¯µ•Ä0s?Ö|b8Wd5?²{¹¯Ÿ–?ÖXI`ãî?®¤‡
[?Ê£­F£Ô¶?¡·ãxI»?Ò¤M«âߗ?®kôn›?àíØe›?¯t
ÖPj4FGL J1303.1-4714¿îêaÑ3íK@/,e@ÌxêÀ;$zØä2DÀ<×ïÖ½—@?$š"v?ü)tˆhî?ÓÅá @è(?çruÓÁ³"@l¨ýº«b?ôÿVø4Y¤?î¬âžž?àdÀÿß¿ÜGüN¿Õ,HÓ
¿í߯Þ)–|¿ïü2JÕç(UNASNone?ÖV3,'?ąš¡ãÑ5?੸D8?Èì>ð^gl?ÁNs=aÊú?½5ÇÑèX?ºúÕ¥ø?¿±ÿE|´a?ç4¥Q×?Ë0k"Iút?Ų‰¢·)?öÀ#yf?Ô3Îó™w5?µ»'ãw.?àdŠÀwV?¸)e¯$´Ð?Æ7ðô;?§¡ƒûd;?À\€3.½Š?§šé4N
®?å G¡†Þ2?»Àþ,L ž?É"aFµÉ®?³&ï_"4FGL J1304.6+0539¿åA—P$kÖ@QÂÀð À:çï¦ìhÀ<"®‹ÜB@£ÒW%V?þˆ×ªva?Շ-;!"$?àžÑç¾Á@}!"Î~@·ü—•³[¿ícƒ'ǁ¿¯^L€PJ¿Ûö î¿æ>$}㰔¿îxùæáK	¿ìšäó4?£UNASNone?é]Nu5Ñh?½½Ó:L?œíP+ad?•
ÕubˆÏ?Æí%¼Ë?¼Ý³äÇÎ?ìäªâÕ
µ?³ °%ñ¥n?š†Q›<?¢äû+0w2?²9£0âÉ?¬^Æ0S}?éûï+?ªgÃÇ»
~?µÃ¢xÙçf?œ§ðë',?ÁBaO¡?¢_ %'iY?êØiP'´5?¤8³Ÿ¼Ÿ?¤3ߤ©ä?"|%ᶭ?¿"Ŭml?¡Ó2~4Î4FGL J1306.3-6043¿ïþ6¿ã7ü@ÊصýÀ8kÚÜZ	À;"KâC@•û¯
t2?ü瀭9Š?±=z	3?ÝXʜpäo@)ð$p!Ñ@ú F˜7¿Á"Ê|æZ'¿¬\w`o聿Â1ÅIö™$¿ÝM1a!.¿êŸwßµ‡·¿î»úýŒ³,UNASNone3FGL J1306.4-6043?ŽÅa‰P ?,ÁCÃY?ì(jêð??»'¾AOh?ºãü‡Ê[í?¸ßÊ$$c?zhµØ|­?‡
ýˆÏôV?è!_¤½{?Ê2¬¼|"|?Χ;ÄÔú/?Ê4õ?³ù´{µ3A?££2»t?è¼Û¶··?°ôL'¢À?öçFˆ?§¨#¥´¯?q—ã'c§ß?`Öa'дY?è®ßË۟X?°viŸv
?Ì·Á´~e_?°G9wZ…4FGL J1308.7+0347?ígŸSgC@P'˜ÜÛ7ÊÀ:¤''%ߎÀ<1ìVu@t1ñê"?üÞ£©½Ô?Ð*¤CkºŽ?×ØJ"]?@_"YÒÚ@k‡ÞY[?îT  ô×®¿·]
½ô¿Ê˜\©#O¿ããBZ£‹¿ì™ V¸¿¼¸ÈúÃUNASNone3FGL J1309.0+0347?ê»QÕäò$?¶¿êHfÀ?¢LDÑY?œT¹˜Ú5)?À§ wá/?³ù€T¤ðÈ?íRìáÛîã?±!¤‡«@,?–òºˆ"¿? 'ƒI¾ô#?¯WԞ5Çc?¨}õæŠ?ç"TOa
?­¿¨R‹aR?»Ñ¢¡Ž<º?¡.—žåü"?ÃÉÝq´µw?¤°+±¦'Ü?ì˟UF?Ÿ†¨±d-ì?§TÅñvÐx?"ZÙË錠?³g@›¥ž?•¬=²H>ã4FGL J1308.9-5730¿ë7`;K|ø@&ôàM/À:Ž 'F¿À<{æ*kä@—"§Šs?ÿü€ï~¨?Õ)ôzæ¦?Üxù!¶3@¨–2æ@¥¿p÷z? JAòh¾?ì¥~tz%`?Ö­Ò HÊÊ¿ãw?}ÄQ¿çæ!‡+¿ïÿž±0UNASNone3FGL J1308.7-5738?×<|*µ?ÁtåÌCÂ?º!­LE¸#?²žxãírƒ?áŒAhnv?©<bñö?Ýõ4öÈ´ø?ÊѤ¡·?£mp7¾À+?ªÛÈ¡œû?ߝ?s?ɗ¾€i#?âá94È?°S·&€ñ?»]p'? $`½Ë?Óf1öÁ-?«_"©.Á?æ/r=/?±¡#"³˜?£Ñ¸?‡s?–Ç®IƒŒ?Ñ'¦ãô´?±Ç[Þ4FGL J1309.1-6223¿ïÈAo.?Ùõ7d›5%À8âŽÕñÀ:é@oUxW€@ÃWEa3!?Àø:8àò?ÚzÁÈó@ÔÌ?ß ?öˆÇͱտïô;pïVe?ïì´É Èb¿âÀrM'À¿êÍ»à~í¿ë'jxÅ¿ïÿ÷Ò4ÛUNASNone2FGL J1309.6-6230c?Ð+âÜ?ÖCÆ+àZ–?á£dl´Ùö?Ó Ë0ÉÒ^?Éd$Òq?È7ân`#?‰þXœÁW?‹æP@Bý?Øü7üÚ¥
?ÎWÃĺ?ã;¼0:v?Î#®Ø4Ñ?¨4ßòáN?–n_™"?ÝÿP
ÿ¯!?¸œ¹ÿ e?Þúö¤'?·–Ê^zñ?F¼æ~jÈ8?7Qš­?Ú,Ehœû?º¢¯aFá?⺺£¬Ð?ºžºyÐz|4FGL J1309.3+8035¿ì÷Ø#à@BALD|0ÓÀ;*qgKiÀ<xÓâjÃÃ@y7OË@ÖÕ"õÎ?À°àÝûÉ:¿º÷Tføˆ?ú.Æݟƒ?÷Od¤šS©¿ËÊõQÓ²¿â¥ôñ¯e¿ì˜¦ŠB䁿ćœDCÒ¿ë†lËÛ5E¿ïÿ••_xUNASNone?îè©áDO™?£
þÇÉ ?‹¨=6Í"²?‰ÓDxÝ~?•¥<{"?¡+þ£YÌ?í·›ÊB?¸*^þÒ)&?œÞòÙПL?°"'-ŒØ‡?°'†põ†#?¨ˆ ×o?í!ìP 8ß?›œ'aþ!?'D:ÇPP?†§`µ£oË?²oLlLdô?—Oxؑž‰?éï}÷Ú·Y?°ÂØ'xÀ?±(í¿Z×}?¦¦57Ö?¿["Ïm´?§ñ"/¸ú4FGL J1312.3-6257¿êÚ²@âüÿÇÍùóv"ÂÀ8š"O…yQÀ:YÔQüL@ (~oÈ@¡Tÿ5Õ¥?Á÷ZjÔÌ?Šƒç€­:@I=Ùb·@C›`C¿ícþ¬Bê?ï(SÜ '¿á"æ".¿æS®h]·k¿çqß
¼òd¿ïü"à՘MUNASNone?Ë-^¾?½ÜnFeà•?»Îxçï+'?»'ÓœL×?åºÙ?ë?Åocs?²UGX à?²}B"™?«k$§ÏP?²þÄeºfè?ìäÊnð?»(Aù4ªˆ?ËöŽÁp$?­gNi½'?¾?Æ[z°\?§öØÀ"?åp‰àMì?±dûE=ªC?µŒ¼¥5Í?šžÁåˆv?«¿-ÑH?"h½»+³?ë'o˜‹l2? þŒ;­4FGL J1312.6-6231c¿é´÷UXïR?Ï!ٙŽÜÒÀ9QTsõ›"À:\Ä"Úœ@±öÃkO.@üØ:¿¯?Ґ`
à?Ü;\L‡@±žs.?üYçՑÂ`?åk¢E9Åô¿âŸ=ÙFX¿â1e"n"Þ¿âÓiÔ¯ð¿ë‰â!GÎK¿ì5?|í'UNASNone3FGL J1311.8-6230 ?[æYüû5f?Y¦wª?"ÕËåí¤?"qNîo×·?ïK^sÒÐ?"¼ƒ¡?¡
%܍É?¥?(;k?¦*òÌ	?¬³Ù3#Ž"?íŒ~uþo3?±ˆ˜|Ž?µïpŠ_?''Ms8ï?È»£	¯Û?¥ëÛEËg?ç<ß''½?§»L±.¨?xCRé¤Â?m2jŒNßê?˜xðLÓs?‹@½wÓþ¾?ï]'ªQ3?	…ZŠV4FGL J1315.9-6243¿á'g^D??Œ¥šŒf]áÀ8rãËìÒýÀ9ãûó+g@Øçk´"@jZíŽ?ÃÌMß?;I§hå@ýœ¨?ãG_ºü?ämªþE띿§Ãހm<ˆ¿åwu³
"¿èœX@2õ÷¿ìPޓɡ¿æR£`—ÅYUNASNone1FGL J1315.0-6235c? û	ã2K¥?¹qÆ:"Ó?á·í¬¿D§?Ò"µ'0K?ÚpÃj-=?ÑÙTB@šÇ?Š·þþ¼?"¸N›)%®?Dz86¾?Äæ>吕?éÓ[Û)ùî?ĕ&/YÌ?¯ëŒ>±+?(÷ÌDé@?ÏÄ«$Û[¼?² T'¢i?æ†~=ÿ?²$[£œøï?;aäú?,–×^«D$?Íp¤¼p¸/?°~A‹D?è däÁ•t?°~háoN4FGL J1317.5-0153¿Û to²_@N&ìAÝ"À;DDfa]éÀ<ø0À'+ç@"¶'MÊä@Ôxã@¬˜?ÑùcCFPÇ?éizi~@}¯li¶?óQ½ØP:¿ïÿûÞ]Bü?ïÿØBKÔë¿ÐgbdÏ
¿é[O6Ÿ¿í"}¶98¿ïö¼?5õÛUNASNone?¼VYILç¢?ºe"ªRŽ?ê÷¿>Zîs?Á	Ä֙
l?§×Y‡·I‰?®3cµ¨$?¬~•¹[Mú?·Öß9ÜHt?ìTÖf+s?Á"ྜyy?®4 Aúá?¯Îì*à`%?ÎJß4k"3?±œ-?›?âD"¹i?µeÝÀ…£?ȤÈYE–'?¦
.+«?…ž
ÏRÓ}?r39vp2é?îÖÔ[ŸEÛ?•sì÷Ɔ
?šVm¤mÚÐ?"‹UÒ¶Ü4FGL J1317.5-6316¿Û<Jwâ)¿áÄ* vmÀ8àÛÿo·HÀ;Ài;'@ÄØâ"Å@Ac?ÁÌm‰gÈ?â›êÂ+35@XÞô½²@Ì$'óÕ¿Ò¾0×@¿Ð¯ª}¬¿ËÈ©¼ýKñ¿æӉX=¿î<ƒß1i¿èPž¨øUNASNone3FGL J1317.6-6315?fæó¾?]_rý¡?ê~ȤlªÓ?¼2Oà?§u?Å©A¢
Zu?»úìÜÚßø?‰;=U_¦?iI(èI?àÞµ'?ËrN9|ª?ßh­³Ï?Ë''tòÐM?™ÀÆ‹ÎJ?ýî~E?è`&Y8q?±á¼¥a\7?ÌNf¤‰¤u?°ŽoÀö;¹?ƒnýh­Š1?gU<ïžFÏ?Ú*ò²)"?³÷ÇH¦a@?⨮'5
?´N²yÙ04FGL J1318.1-3937?éÕw÷f"@6óNÒöÀ:O!Kª"~À;ø>ü•u@¹:"úžA@¡{j×?ÀR‹vÁ¿ºº¢Óª?ô&Ã$º@ϊxis6¿è€zC'üÇ¿çC{[¿å­Á±ç¿éEP6y8Ñ¿ïþ3ý]ŽQ?ïöW_¸LbUNASNone?ï¹Ýeð)?…[â'¼+2?u^¾†Ìœ‡?~Z§ò?ke=E…?xö®ò)â?ï#Ù=eY–?›M§¼$Ú?h'¨ÆT9R?œ‹O?˜rƒ:ŠF?–ÞzF2lü?í¬se{Î?›uÖ%²dm?‰æ'¤½w?€°e;üQ?®¿$ÿ°T?—]g	Ý?ï…Ý?çÍ?‰øAW>Rž?o«.êiSD?e¿{#Ü?›™ÞzµÜ?ˆ+'Eþò4FGL J1318.3-1148?åÐ+›±™7@IBA¢a¿8À;8P©fÀ<þº…¢l@ °u±²ë?üÊØÞ¨—?ÌjØó!?¾úš ¹D@?õyç='@QŒõœNÖ?îåÑ0é­?ëEÅ.î*?´OÝà6r¿ç˜S~,Uɿ̙%•æ±¥¿Î•#éTqUNASNone?îpTÅ?? Œ3iº?]ÿ™™"^?Uûë,^?¨
¶âÃJ‡? jî:n?ïY:Œ­ø?'D¯#Ë­ú?S¡ª¸û%¥?c9,zÅt?"£þڎ¼?ð2U`ѧ?픊(N­ú?•·Áên…Ê?zX{"!ˆÕ?lnªØ#3°?±¶'Hw©?"­錈Ã?îR™áb¿?•h¸·±}?r-Lz Û?n+£Ë^ý?¨¸Zô`?""ÚW|ó4FGL J1318.5-6352¿Ø®J«¿ò¸LH
À9ÿxǑúiÀ;
–}…fÝ@!1{{vn?ÿ܆铬ñ?Ò‡B)V?È'SV\ÿ?ñõ¿Ÿ½ 	?øVª0À'¿ês.0D?èRÔ¨ù¿êę!¥¿âŒ aßÄ¿à¢*aÓY¯¿ä²@¯rŸUNASNone?¢`lŽÂ΢?›÷%ô^ó?d%Ó𺗌?`ÅònHæy?îÅÓc#?œ¼Ž¤¤ó¹?²×ô
MÌý?²n\ç?lM?¢«4ºÔ.?žeœwëâ?í&vу[?´ºOåÝj?ʺÝ!j#?¦@ ‹˜U?±ï0ñk`m?•ƒ59cʤ?çb™¹h?§ ùN-8??´@'[z›?šKäB%pã?öùÊã`?'©b:p=?í-hž?OtŒ™G[4FGL J1318.9-4556?ïö*qe@0¨àP7PÀ:kÒPšLGÀ;ɯe³¹@ëÙá³8Ò@
•Ât"6?×n†›e!¿ æÏ#á~?×ÝلÁg@Õ(eú±?ï==B€®¿è;/`Àµ¿êD~d^¿âÔãâh'¿á,Ãã?l¿ïÿùµc#¼UNASNone?ïk–Þàm?¡fA¸eØF?rwJÁ°y#?n7ªË³?‹Þ¢ç&(9?¡,p·}ôÈ?íY…
Y?±ÜøWW2ç?ynÕ	˜kü?ˆüGÚÙ½ª?±îF‡°Œ?±Žsš{#?éDT™4Í£?ª(í ?£=éj¿w?'ÿáU'¯!?Æ3VR"?§yÂÀHà6?êš{Ï
©?¥Ê=™ò"?Œ…
5qÞU?zÑG4\?ÃÍÀ œ«w?¥KW`/4FGL J1320.3-6410c¿Í'w'¹4¿÷£ÄzÀ:ћh¦³À;cp£×
=@V%üi@·—Ù¥ù#?ÒO/¾¹¸?ãšb‹»`@ãI{t¥@žtGP?¼¤Eoóe¿Ø®ÿÿdû¿ÝSV>PοèöуòÖ¿ïÿý¡UûŠ?ïçÚÄç%UNASNone,?°Dö»‹?ªˆNŒ=}Ž?°@DCZiU?¬U•;:MÑ?ëïX 2°?´Ö€·X={?È/³wë"?¶øDø'ä? {pÍïão?¤OO\£{?è÷=C?ÃF¬YG2?ÍQ®­3Ö?¬W÷ht.ê?Ã¥Á	ˆç'?¢êQ€+ä?ãÂ$9òy*?¯õcÁô?ÎܳÁúg¥?°ò«×v×I?±nÕwg_?™iÓZ?A?æø`"'Ë?³0\Št84FGL J1321.1-6239?Ÿ&Ï6Yd?oÒÃ(U¬À9F&yçL«À:=­P/Ã<@Cïò@Ï©@›çl‹C–?ÇmÍbôÁÞ?Ò7Ý ×ç@¼4 ˜ü¼?ÿ|ºñXw¿êö$Û?ﳨ~cÞ!¿äOÒ`_'5¿æ?_´Æq¿ì†väÝ¿ïÙ2ÁsR]UNASNone?zO3Aÿ±ø?qÀ,%s4À?§Jn¢ qZ?§ÇÈ.¯÷û?îVº¯Yù‡?¨äWÊøÞ½?¢ô°áñ°3?¤‹Jƒ[Ó?³sWõ¢?´Ã¦‰ÑÝU?ìo&æH?¶È#qçæ?µP»Qo|I?ŽÌÕWÉF?Ä\š©¢?¤F›¼)!b?è>¦?¥´B-:B?'7sÂp?"ïðӉH?¨oWz¤,?›ÍRÜØó™?íåMqªB=?¡*"0¥-é4FGL J1322.0-4624?ëoP¿Nù§@0!y[5°¼À;¦v îÀ<ah#ÕÈ@õÃêûáã@ÿ$7í­?×Äzb?áƁŠY5@ÒõU'"@†Ùû3'¿ïö!Ÿ·ë¿¿èJ ˆK>?ïúÕÔ&]¿àwÍaGBµ¿èÝêa2Iÿ¿âG롤*UNASNone?ëübéb^?´wõç,û¤?œ¸¸+Šv§?˜ÈØøå'?¸îÁÒOg?²%ÛT™0?ípšžW|?±mí&Âþ?í	¦H$?š˜t"á$?°}Š^K!?¬mQ›im?ê¡;õ;A?¦L¿Žgað?¦†œïe+?'nHG–eg?ÂÓÔQÌñ?¢•UP½%B?ꔘや\?ªzŸÿ åç?'±‰AHè?‹wfYõ+?ÃwkIÌë"?©™ÓÝÚ4FGL J1325.3-5413?ïò³L"N?@ ž2~ØM4À9Д®xMïÀ;nS™Û@ŸOúi=0@¨˒:*?ÀQii¦î?Ð!û'©@ëÇ~¯2ˆ@1õ桊)?âìv Æ3«¿ÍMõVXÒ)¿ä=1NV¥(¿æ´äv]¿î^? ÿ¿h¿ïùÁ­UNASNone3FGL J1325.2-5411?Ã{·P›š?µu³^P‰Ü?™Y¦ÞÓ?·?Ìxñ¤?æz»ÂD¦?À_­CrÇK?Û
‡¦#?É	³U?¹ä÷/Ֆ?´§Kj`Xÿ?Þjµ3'ôX?ȃd.y¼"?ÖQ¾'ìáˆ?°Ùt½Uç'?ȨéìÛÙ}?§‹-Ôe]à?ÝYÌw¥1¸?®R" n¹?ÚÏÒBMX?±GàÕ
W2?½ÙÐðD£å?¢QúJ8Ǽ?Þ|»ñ¬‰®?´‡d½Gë4FGL J1326.0+3507?éÊ`!'Ã@SǘJAÀ:à=ûäÀ<Ð;êŠM@BúÑlð@¯_ü¿ÙŸ?ÄR†J1|z?À
W¬dM?ûL'"Ғß@!ü@­Å?ï4ãlK'µ?«5〇=»¿áËË]k¿á×>–¾ž¿ãúQjUß0¿ïýí5øàQUNASNone?ïz(ÖÃE ?®ðô×?X¡R÷oÄB?tFZÝz?ŽaŸð@¿'?¬¹]óì±?ï´ìW8~—?"6¤Xp°É?@ÜÀV3?Rd^>]h\?Ã<qÔU?ƒ;!=±M?îøT·ÏI?†¶'ŠØ?lžíÅ?\ÃÀæ¼ñé?qõCy;¢?"¨˜7³Cð?モº.TÅ?h n±?e$1¯Q&Ù?Tg}¿øQ?v$
-
Ê?d9š¾¤'4FGL J1328.4-6231?辝 [Í?§Ë@ےbÀ8ÎÍÐØËÀ:d3çüÔ@9´ú,V@ü``'çÏ?ÌŞÛô2?߃>ÄE@|h½X»ƒ?ô#Ãy<
?ï°iS?Ã~.Ú²¿ì!-Aª¿ëÕÕßðëæ¿ïu'Þ—$Ÿ¿ïÈzη3UNASNone?£Î¿øB:Ž?¦ŽAp{ùä?ÄÊ®'Î?Æ	?Ï<?éh_û(Ó?ÇÔڍæ?¡Ç–;˜?«ê"f"?ÕªDtn?̈sÜ	MŸ?äd"r??Ìuì@Ã?Á%SI?¤SGN~¯?ÆâòQ±ãÖ?§ö˜!G#–?åæúÐy?°®Ô ÒÐ?t·ÈŞÁ?]£èl«& ?ÝoÍ|bº˜?º—†"Ch?ᩱ—w?º¤}]v¿4FGL J1329.9-6108?îsˆ7¿?ö&Ks›ÙÀ9œ§ktÀ;^iŸÖÊ}@Ù؅½™©?ÿà,%!øx?½ø+஁?ÙÒüÇf[@710ýÏ@®€™B†¸?í½ÚÁ'ï¿Õ™0þz™Ï¿Ó¥!ÂÈg¿ã¿YG¿í-¢Ðzw¿è@<›'Á^UNASNone3FGL J1329.8-6109?˜¼NOðÿÓ?"¼wÔ¹¥˜?émýxE!?ÀpS[3?Ç0€SÀˁ?¾)
~'Ì?œÒ,]Ì ?©…;"(`?Þ1/OvJq?Î×XíQ˜?àÖ÷'ìf?Δ‰ÜNm?¤‡Žò!?"WC5 êÿ?éE‰¨ã›¥?«"w@¡ñU?ÅÇõøµ¥?¨5s"ˆé?±Á¾ìžðâ?Yôvi??ښy&šc,?±)˳†Î?àz‹ðN?±º¿hšîV4FGL J1331.3-3818¿ì˜ŠÛD@7ç†
¢À;›í0ðcÀ<zÝ¢w@€?ÐOŽ3?ýç½f?àEw¾}~±?Ò€U$õƒ?õYžfý@µ/â›Á?ïœÒhî#¿é­è j¿â–-žž¼¿Î±£Ñ€ç¿ïhey×\s¿ë_oÒ UNASNone3FGL J1330.0-3818?íýØü㈌?¥«–N›þS?y=³ß£õô?v4ZÞH·o?¬ú¹µÒøƒ?¤ÐþÔ¸÷??în[éF
å?£Ñ2½ÿê?vgÇ	î$š?'¿Õe©[Š?¦MHŠa]
?¡eݐn?ì9I2G‡?ž¢‰6öÿ†?šY°"l¤
?ˆ¯…UlÄ°?·ŸJgbšÌ?˜°1¬\?ël'D=iL?¤l÷^õª?{ˆüXCxD?{ÐÌ|káÁ?ÁqsH??¤;ÂE^ý4FGL J1334.1-4154¿íÊëu¦Â™@4@Ùè>B[À:`˜I7wÀ;ýːŒªž@¸0d÷¦j@é̂$2?À˜PƒÑl¿¬6ð/U?ç¡»Áâÿ@ɘ
²¿ïðG€^?îqu‹u•¿ë\dŸ¼ÉJ¿âj´>`ß¿ÙyÂ,_Ú¿æÒŸ½J#UNASNone3FGL J1334.3-4152?îó™ÊJŠ?ª!UpG^?'k²€LÃ?"8Ü}K?¥í#4õÛ?¥ZY}SÏÆ?ïn½-Š^?Ž8Ó֍™=?U ^"¨?g‰P©
šÌ?ÔGdei¾?‹×®°àS?éçÖzÛ ?«-,1ñí? ¦§zp"?~Πæd?Ä6ü8ìm_?§íãŒa4£?í³¨À…?"BA>@+Ö?€ºŒEÅxN?rêʟ_Øà?°P)6±LÑ?"»Â^yŒ4FGL J1334.6-4435¿ï÷ê,"|@1šP?³t6À:OÜ»WZÀ;þ†
˚ž@HÂÁ@lÇß'Bd?ÊWvßZn?ѤÃ,ºô?úßú Âî'?ùJ¡¶×¿á§úð̆V¿ç­czù›b¿ßí´ctn'¿ípÜá¿ÝwGʙ즿Ð}U–4ŠKUNASNone?ß͵ƶñ??È+Ù@·V?¬11˜k,?¨Bû
ï?ܱ¤\?ÈUåÀ i?èðh$Ê)?Ä¢õ"%?µ$6ó´'?¼
ë/DÆI?Á¬WT"ý?¹~ZC©Þù?ä.¾"€'?°Sé`È?½'Ý.?¡õÿžÑ•C?Њ=Ìuô-?©ƒ#¼è^?ᤫBå"Ú?±åÃQ˜X?©^õ×C»8?™U>$w?يʿMBå?±®½p~ö>4FGL J1334.8-3856¿Þ«ßÞ2¶ó@7("Æ£½àÀ:TqËõ6xÀ;í½îãx
@^¬ÛA@0!ùO×?ÁÀâ]Ø£¿¼jØE²?û­N'D?ú/}F'?ïôòñ#Ä*¿é-€¡{k¿äºïÀÛå¿æRuþ´ÑX¿ïöö¡²lÏ?î3Œ>½*UNASNone?î¤Rd3gÂ?§Ò./ghß?›7ãJ"d? ÊkÏôg:?=Ð.ÿwU?žHÓ½õe?Ꝛœu?Ő{yàg?°ö'±"@þ?¾
ŸùNù?º¨jÃ6&?·BûGþé«?èý߈qÀ?©‡´ùՋ?¯Ù¡4½C=?§G¾°R?Ä'	®â?£5ZÊöW4?èÔd¦å?s?±*»¥>?ªl%¶\\?žÝÆÜkÇÒ?ÆhÚýk?®˜Ñ	4FGL J1335.5-4546¿ïÛ·"Í?õ@0ií9SÞ¤À:Ao.ŒÀ;û~ÿº_ã@÷ `ȗ´@ßݵR?ÈEF³î…?ч¾û¨ØQ@5]¢r†/@ÔPXÝè?äčc*qÄ¿ÖÛh›õ¿_¿å"øD÷¿æ"6 M}a¿ë½ËrY¹°¿ðUNASNone?ÝjHþ@`?Àëþ‡Îì?ˏà¿g1?»~ø½Æ5Æ?Õ¥³"?ÀÁd†¯¿:?âŠ`ðqŒ'?Ǚ"‡ÊŠe?ËKwb;ô"?ÃéºCö§?ʋÛýÚÐ?¿³­6'?á…j·$?±®Ú_h?ŧ¡Ç#™?¥HÈò"^U?Óa¡Zæÿí?«NéÐ?Öîˆ*å¦?¤U>Ìë8?Êx[8ÿ»f?¥=Ǐðäü?ÛÕJHU<¨?©GÜñ 4FGL J1335.6-4052¿ä¡Ÿ:Ôxy@5;n.±Ä3À;^bMÒòÀ<…ú¯^&ý@!ì¿	ª@Óª6ŸÏ?Æz}ʆ –¿ÁÚèÄO%?õ-§¾Šà@ƒçÚ«?ïø˜,²²¿ìCË0ëZ¿ÚÌù"@F¿ï/<=Èã^?æÐ;·f3;¿¡Aµ)ßUNASNone3FGL J1335.2-4056?îÖÁa}å²?¥ÐcWB«?H†I§%¨N?S.h
¼@5?¢1ÐÁ…<?¥æ!>â?ìö?cª²?Æ\¨<bZ¶?‡ð‡P ?¢†ËàøD?¼R=ΖÉ?Åu®YT9Ô?ìÖEwòfú?šþïë&ä?€ý¸'–B?zAþ» Þõ?·.0iZ•b?™‹~«\?ëU¾?µvmåOKƒ?QÀ èâƒj?`ôýR}ù?Ø
pÙïý?µxŽ­§Ë]4FGL J1336.5-4655¿ï¼iûúÀY@.}â:óÀ:Akn
#ÕÀ;úž#lÓ@?£v'-•@éZD4"?ËZX¦ŠBå?Î[Ähû?ÿÓ8§z¢@ú…"áQ?Í&ý…Qc¿ä,È`›±¿éšãEµ¿äAÃ^¹ô®¿îq‹'æÎ×?È}+å6%+UNASNone?ÞãQæ(3Ä?ÃdðäãŠ
?³¥ãjU?¸Ä0"][?×Ã(Fæ?ÃIo+cj?é¾¼ÔÏ?ÀýçGÆ5?­ÑT±£S¦?±àÒBiß?Á"¦Œ£×Ø?¹™_9Ö?å žÜg<?°­1tŒ:"?¼«ÍrC›è?¤}Xh>™?Í'ÕA?×?§  ¡öP?æÀ@Y?§º¡¹µï?«°¶`wL?Žú÷ÓUe?ÎúVG°È?¥ÄÏLG3L4FGL J1338.0-4159¿Ü"R@4
šÃeDþÀ;
ÔoX}À<‡µ¡7Í@  ÍâK ?ú²?'ÌÎz?ÕòÄMã
?Ò¥kŸ`X@(‡€'a—@Ç°-YÕ¿ïöÊÍL'?횣"Ôæw?֓åDè½C¿ß5î#‰œ÷¿ÍK€†ù¿éÒ%œq».UNASNone?!›&û?$ìê@,K?Pÿ³GÞ#Û?QÑo¿¨â?Œô0:|º?Œ9½
©{?|Ø­A?9^¼©r¦?G²F´ž–?c%9D1Dè?‡Õif?Œõuë?ídç›aö?š×6¸Ü>]?øl{dB{?v1YqŠ*?±µË3¸gÿ?™yÝ­Oâ?ïV…ଞ:?}¸Æ^K°T?@-mîA_P?7öµTܦ?"­Øzú-Ç?}…"Üû%4FGL J1338.8-4509¿éóÂ"µó©@0çm"BJ'À:·)Æ¢ç À<6,ém"@MCtôɖ@ËHûòTF?Âü¼Z
è?pý
~Êeˆ?²y=®ŒDò?øà‹ÓÞ9?̙ŽŒ"Ž?éêô€­¿ç

Ÿû³j¿å¨šÞ"Ô¿æ60ÞÅÕ¿µ8äx0JUNASNone?ëîѨ6‰?´ð#ʂðX?‰"kU,%Ù?"Eâ؉¦?½XåSªVÿ?´[¼n?ì¦ô1ç?µqÙ -?Š­4åh?'ý
{|?·y±Âă½?³ó{œlÉø?ëéŽï[‡­?¡(€ôöÂÊ?"KX+/Mž?'ŒóǨ'?»à²zWï3?žD5AHñ?ç–Ó5û"J?¤Jµ8)?©s3x`A8?"³/!Û^‹?ËGæIûf?£ál¢Óvÿ4FGL J1343.5-6827?dÜEÀHŒ°/À:ËCæÝõÀ<,Mâ"s@=;"@óÅ¢6 M?×*Ÿ[$"Þ?îÍ~d^N@f"»ë@;(ðÁ?íÛûß	s¿ÖAcAî·Ù¿ä(³GÀˆò¿ï춬Ï×C¿Æ¹Ä1r¿¿ïá½õ™t±UNASNone?ÔdéÃĒ?ǵÎHÌR?²Ð—‹Ø ¶?±e…: (Â?ãsxŽ# ?ÈE3=§Ûï?Ð}Œ±¤w?Ê1G²Ê?½É˜,j1?Á݇Üâ¿ñ?ä¤Èd?ÌÖ4V?܅*ñ)b?°qߧEċ?ÏÅÁ€Õ?°Xâ§tý3?ӗôG÷³?ªØËâ*4Ï?Ôs‡(}?¶ƒ¸S¤Õ?ÎXm%vzÇ?À'Üʦé?Ü`B[¨ ?¼iM)·4FGL J1345.9-2612¿êŠ-ZM ¿@A‰:'£SÀ:¹Y×êðÀ=£.mѕ@©t$j¡@Ç<t$•?ȋË:PˆÚ?ïþƒ~$H4@&\âY&@	>èŸf7B?íPŠ\õ¿ÚrÃ×ZÅH¿©–Ú]À5Ì¿él«úÅ-œ¿ïÿþøþ"?ïj8$óTUNASNone3FGL J1346.2-2608?ËҜ™c/?Æùàé£?è˜?IàA¦?ÇúO®ûü?"فß,±æ?˜?9ÖaÂ$?¤6#B?¬?¼‡zà?í¦ÖƒÞŠ?¶>à†'k'?ªÆ\t¯?¨WE
–?ÑQ´ÚÁÏ?±RË=׌Ù?ãíO9'?P?³ÊxÜÊO?»N²ÈnÉF? F4¬/?³j6Æ%T¼?¥^Á*3/D?ì
3e¢já?¯¢}›U:e?¨ˆ\Ž¨p? ÛÀ™4FGL J1346.5+5330?рUw£@NÜz¿¹¾ÓÀ:h™î˜ÏÀ<ž))Äõh@œ³ì+6å@ö"ï¾i?½–Öñ"×?¹6w‹QØ:?÷W›ÈH@§¡§…§?êà^úâ4¿æËÔHµ{¿é€NÚX¦Š¿ç!ßeUÅ¿ïù¼º0¿Ù&ðކßUNASNone?ï+WãO§?ƒ1J¨'?'C¿ÝH?€Æj5±&?tQÍÒØqý?oÓÅ·"áB?í«¹äq?¯Ö}ý¦«?'¶Aœý˜È?Ÿg
3F?«é@ïßl"?¥:ºö0Öe?í'Ƶ™ÂH?"×òéM¨?¥ñ-¾°?€$^uŽO†?®ÙÁ­Ìü)?Þï$Jd?íR""ƒç?©ô?°s³tñÌQ?›a}Úñ!*?"ìßȈQÄ?{"]+Gè4FGL J1348.5-8700¿áh«©ÒÀ8;*'ñ¶'À:ˆ cLÖrÀ<2
˜à66@ô%8Kv@Ô¼÷"?ì˜ôX,¿½­‰:¦Äû?Þd¸[¦™Ý@	D&{Ÿ^?Ñ''?X¿ãáÚ{9¿í^lœáL·¿ïþÂþ—Ë
?ïñhÃ7ø•¿ïÿ'ö֌UNASNone?ïƒÐłK?¼JÄ Æb?T¿9=P?'K•›‹A™?ŒsíøME¤?»o—gèÛÖ?ïrr'%?ž	±Œ?p?Vs.Pæß?x+"øa¤?F̎Ȭð?›Yú$Ž	*?ìvê'iú+?£-<èÈÝ?€	؆€?13ƒêç?ºGpcà+T?¢£kӆŢ?ïõs]Þ2	?\±[îYš>Ãd1'"Ò>ãħ{¯¬J?U¶ƒ-o?\½OWÿb^4FGL J1349.1-5829¿ê'Ä5N–f@Rºû15À9'ðrÄB»À;TkJѵ@ÇÏÿZã@ù†üÞãP?ÇSÖö·W?½0Ãj¥?ö"fÿéYË?ûr—w*ƒâ?ïÿûÎBÓ¿àxŽ¡îÒ±¿éñ×HPѪ¿éނö ¿Þòb+‰ò¿ïš¢ãÅ6ÖUNASNone3FGL J1348.5-5833?ԓ͵"ø?Ì*"Øž&?{=yøâ#?––"÷Î?åžô‹|Á?ëèš^D?ÔNöJð?ÄöŠ'ÆI?°gâ/nÛ?±îӐÓ?ãËý?˜?űµGóŠ?ÙÂ-ÞJƒ?±˜óÜë?°¯Ž¦`âª?'R:ÙK?Ü?á÷<Øé?±RÙôXû{?ÔÍìÚ¢;?¬…9à¥K?±9ß^Ë*?™†ñõx‡¹?ãxâVÃ}?®Ã#$&Sû4FGL J1350.9-2757¿Í÷[¹¼û@@ŒÜY1ÊÀ:z(4Òo¤À<Ç]!CG@ÌÆHy@‰@¢\›âI6?Í{±ýºÃ?Ðé̂$2@;#Â|è?þ9—ÒÅ¿îðŠ!«¢?ïDŠ=Ü¡¿ç®ùþY¿á)-÷¿îk½Þrf¥¿ïìœ
!¼UNASNone3FGL J1351.1-2743?ã(»‰?°ú$kČ?È}äÅa±)?¼ÙAZ¹?Êá¼N'0°?¾hÔ0mw?æÒ>Ò×Æè?ÆOzŸo !?ÅOº'NU?ÃƖ‹^ñ?¾Î"d¥²?°Üe P?ãÊÂ(õý¨?±íUM(€?À›´˜œ¦'?¢fÕ\W$]?Сaűg?©üÙj"Ý?ß{A}
0'?­ÐÍ~^F?Ð"ùù¾?¯t{Àú~8?Ðy›ˆù¹°?¨´øøe+4FGL J1351.6-6142¿àԆ°fmP?ÕÃí_êKcÀ7þ§vÑîuÀ9òzƒSÜ÷@Î$ªYZ@(H¾µ²Õ?¶>$'ýu?Ñا¡o%þ@ƒ(ùôMD@n,"Þsé?ì›Æ/#Ùú¿¯¦^B¼¤¿äÛé B*G¿èõ~ò¤M¿í3nŒ¥•P¿ïÿúVrÓ\UNASNone?ȧ÷Ñër¬?ÓäáJUЬ?ᆠLQM#?Ðτu©?ОÃ~g¬e?ÇØD׎9ð?'Ú¶\?é¬?‡PÈRÅ¿?Ø¢àýé?É3•'°?ãc$çd?ÉO'€8?©R8EÕ?˜
¶¤ÿÃ?á5S÷²5Ñ?¸…üÛçüy?Úk
ÒÙ½?·PT›\¶Û?Z	p¬?Hù;=gPË?ϲh!àØÓ?­õژ8´=?èavGƒ?­ÿè2dó4FGL J1353.5-6128¿çˆrn¡7?à´¬Ã˜À9­ê‰v6À:DmŒËU@ !€
+Œ¡@Ù\T"­?ÑÜ©ò­1?Ð¥·_'WÞ@–ѵ(k@_ƒmÞ)ì?ïQ½ei¿Ù¬bÉù³¶¿æÍØÀË◿稊-¿ìèÜy¿ès¥J_ UNASNone?‹_¸sÞã?†c+²~?ŸXߒIjy?Ÿ3Ž™Jx?"ÿå0?¢ãº™ƒ?™yÌ®=?¡Ë«Ü¨?¢D
j¨²õ?¨Þ¤ú;žÃ?î#ZôŸ_?¯yD,ÞO?»²GØ$R?˜Ó‡‡fÁâ?Ã"=ÀoPb?¢Ì^:Ú\?çÁ0Fé'\?¦ÊˆÁ\ã?€Æ¿þÎÝ?kÙv4|?š\Ë=Öæˆ?ˆ»ZÚÓ1ò?îéþ¦
X?Š
)£([4FGL J1354.2+0353?çvr¼ÏÃ@O,*^x[[À;]ôiÉÈ6À<®$´ë.¸@ ͇‹z&?ÿÄXŠÑ?È[XjËP¿†¥VøE‡°?ÀÎ2èà~°@9ÂÌÓ?ïðp
TÙ¿æo^݆Ž¿âWʌ€¬c¿ìI!ñ¿Ë?ÔÉÛÁ‡I¿Á•ãšzUNASNone?îšàlÎ? †¨%yσ?`Á8žÌTD?^dž"j¦?¢ÊLXmÝ? &'¿v"±?î°¢£úq?©ö°¸¡I?pšàCô±?†¯}ӗ}?¢ë£y·Ú_?¥µ:dL?íiÖÞôì?–XäX]O?}f¶¥vü?r™"r]Ê'?²Úè<îHh?•SÃEGd?îFŠ"΢Æ?™×œLK§÷?VîÖB?[vßo.;?ªç@B7!˜?™Ãݾƒ-a4FGL J1356.0-6747?Û«PÅUÀÄSK×nçÀ:RebZh+À;Â)©FµÇ@¦¿Ë1—'@¼¬ùÈ®Z?Óˬ¦¼—Ë?è-3¿Ë¤@yl$ìH"?û[9i®ƒ?ïFòbˆ‹T¿Ý½<‹÷p¿ëXd"¿íÁED­®ú¿ï¼~Æ.£¿é—€ŸÍAUNASNone?½,DÑ5Û±?·¡¸¢±Mï?°ÖdÐwß??¯é3Gç³?ê?ªËÊH£?¿–xFÉ*?ÃÇb?F"8?Òä€Æ®?ÍD4éj"?ËYž‰VM?ã½5ÊDM?Ë\ŠÚ¦³¯?Ô¢‹¹~Ãõ?¬eb¨Ã‡/?ÊòoºZŠ²?©v!#©¬F?Ýä<iSö²?±0×ÒL,?³å'K¬Õ?"'®{yZ?à
,ªpz?¶¨qÁ¢)?ÚòB4
Í?´£¯/ëÛ¼4FGL J1356.6+0234?Û4+M-'@Nt*€JÀ;ÂÀð À<Úü›ÇqC@úk­ø÷"@ë=Ñ?ÐmÝvV?éºÅ˜ûäè@ô]…TÖ@ûlYA:¿åÝlÇ©w¿Û É8Õì¿Ç8ÖöœT	¿éŸxÁ1ãþ¿ïÿÿ" 5•?îƒÁ@&¶£UNASNone?ܷȔ4?ÇÏ,®³>'?ÙÙa5þ¿?ÉîNb5y?Âݬk›®s?¹U…8·V?Ö(^÷ª<?ÌÚ͑4S?àȉååÃ?ÏÑ#
þ0l?À}¿~?µƒTzTÓ?ԟª\ø/?µ
õô¸t¨?á;‰rRà?¶Ù½å¸?ÁÔe Fˆ!?¢Vªñ«Š?â.rx:æ[?¹O¡ý%H?Ó®
%F%?¸Jñ7Œ‡?¿ÔB	"´—?¦ªAë°ïU4FGL J1357.3-6123¿î»¯ÀÄÎ?ސpõ³ À8ïåÍNÓÀ:æ	´´¨@7‰Ia@ŠR¹á7¾?ËÛ)†âñ?ß[_!M­ˆ@þª°BR‹?ÿžwì©·¿á$rÀç¼<¿¨}ô]ƕâ¿ÖÝË!Ñáà¿ë·†Ÿ@øn¿îÿãIœV¿èD?JÑUNASNone?fàuf¶a?g	ãåØý?Š±ïø?@QÓ!â?B³Ñ‰?'è20©	ù?˜-´®vé?~…Ñ?¶Pä¹È?µ²›Ø¤Ä?ìuÑû!Š9?¶VFqz?­%õM§}l?ŠeÙ!^?ÇW­LË?¦ªöÑ?èg
¿ä´ö?¨ù"?m¾x"í7Û?_²¾®£Þ?³&»«¯ˆ
?¡ˆÍÔ3?í}jõ!È?¡ø¼FšfU4FGL J1357.9-4907?ït¯ÿ®î¸@(¡™V}»À:ÜþÒ—À<¨Ï—'h@¬Æã#@¿Åäë?ÅÓ\ÉY¥¹¿ >ªhR?݊´cõGë@z²ái<?ïÿ< A¿¿æ…¢×/ý¿ì·¬ª–¿µM`:—¿è*øÒU-¿Þû¶YÃÀµUNASNone?ì.,‹EIô?¶õ3'é8?lÚ(³"Ǒ?jXN¹_?½§Ê`<š-?¶°Ï^÷A‡?ìkË:'?Àæ*«8Üß?i¸Š ¬©?x½[;ïÓ?¿!ÈL Æ-?À·p'óÁ?ê£_5>—†?¨59æá1?'"Ÿ¾?X‹ê?ÃN/3D@†?¦¥'0q?ìòBMNÖç?žàBƒ@?±TM?sVÅ*}S'?¶JÌ^Å?'†ºûg«4FGL J1358.0-7749?Ì	°7À¶"À.Ök\šÀ:{@¶©tÙÀ<)ŸY@J›÷lÞ{@̳_=}9?Ìu´øo½Ó?Ç{V¢ùê'?üû=ÈK^?ø))ò—·—¿ÄÏ8
û¿âs~&÷f¿ç©>RK&¿åãHÿù¿çú¢'ݔ›¿ïÿ/‹_UNASNone?ê+®mãl?·'ͼc?"W	ʵ‰?'/Áp ?ÄÆb§:[ ?µØ¢<(>¨?ì§ÚeÑõ0?´yQÝVæQ?•Çʏ"F?˜'N Låð?µO:-‹"Û?²ñêÁ ?ë¤AªŠ"?¢"ëô­@?›¾¡öžƒ?Šz"þ¬e?»ú‡².Å?ž?葂$?å0Œ'Úüq?¥ùË·ðp½?­û{'òîË?"
›x°€é?Ñßwkë©E?¥

§4FGL J1358.3-6026¿ïã6¯z½?õƖ^¤ÑÀ8"n°'-À:d>XˆW@x=û»ù@‰¤Y=?±XR&"g¦?ÑyYˆ1'@@@&`½?ÿF
ñ/W±?îöø_LÁ¥¿Óîtý­ë5¿ãKíÿ¢b¿èÉf@¿ëÓß ¹ôX¿é3€`°UNASNone3FGL J1358.5-6025?y)亠î?tu~Y?炧9G?ÅÓ{&Ï·?Д}Mú‡\?Äè~?"‡¯?€5ž 1ýT?‰{EQÿÒØ?ÚÛë2¨Vò?ÎÐÙ!,¿ä?âQ3ì+'?Îâ߁áز? Ö?±Ùq8?Îe£†
?æ
ÌuÇ0?´Ì‰Åò?ÑÃpÙC{?³e2–7?eQ²,ü õ?P¾K¹‡X[?ׯ›YÎ{?±3éäæ!7?äà ëÆR?±93Öß4FGL J1359.5-6615¿Ñ;9«·HÀ&0"ÝzšÀ:wŒ 4RîÀ;¤»5˔@Hàø'ï]@yYE³Æ?ÆÅÒG5Ä¿¼·^""m?¸ßw^Ü.j@ú\­U
N?ïôÊ(,o¿æР@ý¡+¿æ'³áÄU°¿æWæ`ǖ¿ËTO£uœ¿ï¤œ—zÛhUNASNone?Ò¼ï=ßòÅ?ÌÛvȏ´?{"Ð_2½?p¸	)"=…?ækBÀQ¡#?ÜÇâ)+Â?Ú{&Òîf?Đ/»ü¥'?mS96'ø?€2ìîX ?â¥"ºÒ:?Äc´Ù0‡i?âL8Ücbm?¯ó;ÀJ´3?¢fþ	:?†ÉŠoR@q?Ù®‡?®kÈ9-7m?åÈZˆ??­œýÉL?w¼K_Á/?m±!´ºÌa?Ô[}Âj}?­è§,4FGL J1359.9+3616?îÖRpÿá;@R5!…Æ~À:¦ªWVþêÀ<"웟-W@+èJ%@§†
¢?ÃٚæuÀL?¬jÐa	Ñ?â%ëoOC@"N0"Þ¿â¹_'F–½¿ã¨"ÿÔò¿êÀÚPC¿ïØ]ÂRö¿î媞ú'¿Ü¿³O÷9UNASNone?ïÖxÕÇëö?—]ÕsÄ*?dÀ|ìxúU?Ž]oIbmE?dÆ­K›'?…ÉQù?}?¢'4ïPó?wW{Æβ?‡k<ÇÕàN?¡£fNT?ŸIŒÑ&¡.?í'ØnÏAL?"Õ¿'Óf%?¥#ÚÉ4õ?}ÕÐåk?¯y0Yž?±‰Å•—µ?î¬&xé˜?L½€[?™Q¨Ý·5?‹¹7ÜåÓ¦?'+òS+Èã?}ŒïZàÏ4FGL J1400.0-2415¿ÕQÌ—Â@Bt§qÉqÀ:B¿ö$´ëÀ<}+é'Ö1@%Ù}_QI?ûÎ:Ufcâ?ÃÝýâŽl?ß(Cëè@fX`f@ŒÀ0Ýž?\X¿Ô¡—Zû¿Æ.·ùVº¿ã[ãU¥N¿í€<›'Á^¿ïË!6±mUNASNone3FGL J1400.2-2413? EÜ,X?™Qy­S"Œ?íVÖ»µ`?«²--Á?ªM€h'™¬?¤-=9Ûy?·e%ÌÊï?³¥î«ÙÞÒ?êfFv)Ñ+?»jüãªÌŽ?µh¦æ‡¬?­oã+Í-W?­TÏ~"5
?•­«EÉ%*?êÄ¿iy`n?¤ÑOm›^?»/œõ#â
?œ{
=Ðn7?Ì24õËA?§PŸU>ë'?à¦×'òáÏ?µL×jÜÒ<?Й6՟VÂ?®ºTIIŒ4FGL J1400.4-6050¿ï2IÀcL?ìóŔÊ'À9·ÓôzùÀ;CÓÀí@l§"W`9@΍F¤ÿÿ?Ѷùü°À'?æ†\㔏@wàmò@ÜòJµ°Ñ¿å>, òÔH¿æ¨!â}ä¿Ñ}Ýï<¿å.	"&¸Ñ¿ïÿý`éNä¿à–
~C›UNASNone?¯O¬K}V?¥‹==£?³•mHºg¶?°šòSâ
ñ?뜝\#û3?µº§b@§?¯aÁű?³¾3YH§?´Àm²¾b?´¾*õ—t?ë‡+à½M"?¼ò
?Çc@p+¥à?§Lþîa¼?ÇßkZmh?§Ž›Cük?ä/U
Y¶.?®©i|÷t?³ÒÜ;çþ?šž¦'€Ò¸?¸.	Gú"?¤*¹ôɸf?êý;†Ã®?ªp«Š$ٔ4FGL J1401.2-6116¿ïZÀETóÍ?ÞQ%ʟÀ9[(5©/9À:Ób¢Œ‡b@·:ööìÜ@ª`üšò?ʗð!:¸8?Ù¿E» '@
	_à:gÛ?övàœià¿íD]Ä×5?¾æ]Â}ée¿Õ˃ÁÁ¿âÎòJ¶Ý¿ïDá±``?£Œ'ìG-UNASNone?'2Áó¬Sj?†gþ*'2X?É|Ù¼á´)?Á²tpÅ5?é3*0Z?Áú\°#ú™?'ǬœÄCX?•Ë4÷œ³â?ÁH–k=i?½÷(¯É½?ëJœK?¾|ÈB@**?·^	¢«î?'š´Ã&T-?ËÿƑ
í¥?«ðoçð´?æM'k?¬Üfå×'?‹;ȪHEG?röªÊ–D?ƛ«§ƒŽ?¬__«?éì%óuû‡?¬^ãQ/(4FGL J1401.3-5012?ïëO¿äd¢@&Aòý¸ýãÀ:SQ÷GËÀ;åF­czú@1ʨZR@vÜB‹•Ë?ÉŸY¢Ò?ÃsÇ¢ìS¦?öO²$ªÚ4@›±vÚþ¿â¡{_ò®ß?ïõ–Ÿê³¿æ¿a>ß8à¿ä¾É¿Q9.¿ì¥Xtá¿ðUNASNone?ìN‹DºB?²ÊMˆc?¥O¤t¡ðD?¢Â3`¯?²ãӟÞuÌ?¯&:§‰–?íM		=Nƒ?´vZ€Éþè?‰¢ ã»D‡?•{õŸþ{s?²cc™ž#V?²[ÖûKD^?æ,Ür¯6‰?®ƒÙį£?±®/H`ŒÊ?—ìNÞ¹#?Îuv'ßq?ªTŽfˆ?êF‡bã?¡ï¸Âœê?¬D¼©>?"Ú?ÂZC»?¿©h÷@Iè?œIÏe?˜4FGL J1401.6-4645?ÝÑt!N@,×`Ï‰@À:_!©ó›À<Á±æ—y@×\Q9®w@æ¤ì´?½x؃å'b¿±=Þ^p?ó{;	ÁIâ@·•‡U
¿¥ò¨ êé¿é
á,ˆ¿é//˜sÿ¬¿àC݊¿ë$®ÖAÀ•¿¦&™áÔpUNASNone?éîü(.û?½ç_ÙÅõ?š)ƒ¬¶¦Ç?[膿LÀ?ÄþÞê<o=?½)×9vÓE?îÙòڎs?¡í°?ÈU?c³Mk¢æ?t†4
Æ?¡%®Í€^ž?¡2j›$Š?ëcøþD¾?¦–"Œ7s?™ÀPOê?‰†EÒ÷?¾p1KqÆ?£9öˉã
?íï©[û.Š?»v¬Ê
t?|ßJ"q>w?i"v2È?­i€íÞïŽ?u´XebÎ4FGL J1401.7-3217?ét§L4¶ì@<EB€®IÀ:½–V;À<x¸Œ£è@WrÜÁb?ýTyð'Î?Õó!à¥q¿?ÖÂhż7S?û\ߺZç@QG9Oó?ïyn‡P¿çl…>õ!¿âãÊ|"¿ØŠYàœ'¿è¬¦Q8ø¿ìžÑÿUNASNone?ïW* ý£ò?ñ…º26?cQMD²?`"ó-u³?'°‰v¢ýã?t½€Ю?ïþᓐA?Œl^,Ð~[?Ró£Ë}'?c´‰Ï^
[?¼é&¢€2?‰zæú"h9?íjÕVn§?šEA`ì?Šlœì;?|
p™)±?±[ÔXîqA?–´õÀöV¤?îíõ¥"ÆÍ?ä~›ž?f¥o׿—ú?Y—[)eG?ŸlTo3o?[^µ(xÈ4FGL J1403.5-6236¿ïØE«bw¿ìD¤¿èbÕÀ9NûH
[À;ži9}@ŠÊ"£n@í÷­K'?ņIÖ©?ï›ü€¿@Žï¬.@ËÔ²IhÕ¿ïÿÝ/ñ_S?ïÿp\‰¿Â©•e,¿ã¼ì™.:¿ïÄaùð†?½•æܘqÑUNASNone?"lÐÆ@e?žòèñŠï'?êvŒIMyÒ?ÂkÈa"f^?Ø4Â*?Á$Z~§#É?‡"ÎyüŽ[?•Ã;¯)§?èð§ßf1?ǖÄxX4c?ÊƐxâžU?Ç×%Jtt?¶žÑv—1?ŸÚÙYÆãm?å&€¨¬?°‡Ý>è?ÐJg##?­:SoÖvë?s &•'2g?g0¢…Aþ­?í!ù\ýë·?§‹u7ì#Ü?µ¶2®¸?¦¸
fªÍL4FGL J1403.7+1513?Ñê#¨YX"@QZ0#̎À;hÙQ?µÀ< cÞÌ©'@A_ˆhš@–•3®?ÌOÈ?—Á"¤+1Ì?̒ ¾ç[ï?üŠQՃ¿ïÿÿ" 5•?ïÿúVrÓ\¿ç' ¤:\¿ãUGá‰ó¿Í–õåÊʔ¿ïÿ%¿Ø·UNASNone?ï!"Çi?¥¼ø'‰?_H®½õ'®?`ÂlëõQ?™ØÜ&ÿ»|?¥'†–±±?ïr¡€5[?H®–/Š?NæI>}"ç?[E@š£&?Èy†k{?ÒMmÃÚ?ílкçXº?–©#@ Y˜?"µÅy˜ïn?w…î$@ë#?²Áy'9?"ÅE°OÆ?îRîdÈá‰?|‹Ù]n?+(ˆ"n?ul§×­C?¦ï´N`Õ?Ž·?­\gd4FGL J1404.8-5237?ïáçOž½Š@!M¤¬ó²À:lÚ"À;癴qŒ4@NMlDvÒ@ˆ¢ù"«ô?Á6F8¨²?Е§œ'›ž@	ŸNÒö@+Å ¿Ë,a‡ÚTu¿ç¼"pdìê¿Ôïʓ6©	¿æÖÜH¿êþz#²Œ°¿ðUNASNone3FGL J1404.3-5241?Þÿ½)¡º?Âc¸:â!?ÏC+Ñ^
?À]Ð>À?Ñ^¬ù']??½šèY?ÙÚ9"F?ÉìüËk*?º÷T9ôA?¸SûayT?ßgñ^<ñ^?ɛ´ì…?ݯHV»Z¾?±¶¬rP?Ëì>ð|M?¬
ÛÓù?ÔZ˜1~€?¨È½¹~?à'7ÆNèÏ?ª9»y¸³?½\-ò?¡Y,µsûÂ?×{9gå¨^?ªã @a4FGL J1405.1-6119¿é¡ÑdÈ<Ö?Ò&Ÿ;š
À7€®I#À9iÞÎW@	¿Bu›c@PŠ"Ràx?±M
NóA?Ñ(6À[zO@"µz»ˆ?öŒ¯˜ß_w?·Ë¼V‡÷¿×ˆï]J¿æ«"zuè¿éç.þL²¿ë'®/RÓâ¿åï@4£UNASNone3FGL J1405.4-6119?pï$3c}?pø×n.{?ɱnäæ¹?Ä"³<–<5?éqÅþ`Hõ?Ä;n¦d4Ó?pȾÉÀ®¹?zff-•?äSbmû?Í"k|~?×*Ç?Í
ЏD?¨w¯h /\?˜œI.ÿ`?×ÜoÆ©lê?¶V·µL½?âŠM&!F–?¶AÓÇ*?ï?½êG¸Ã?
eâp?Öù•ˆÐP?µÂâÍ{ ?䂑Åé_s?µÂçNŸXü4FGL J1405.3-6008¿áoóÚû<?ö«#/¯ñÀ:4äR´ÙÀ;^¤€}há@!¹ÙNehº?ÿ7½¯lj?ϧWGd˜†?³TÐùøT?åóÕº²@ò^ªuÛ?ì‹m¡Ä
†¿ënÁê»m¿æìma,j¿å!Á›Á<¿ÜˆC{)ìã¿ß]©~i'UNASNone?ÃP*†Â0é?µs¯Ýñß?R¹‹¹·ÈÕ?J–ÃuN'œ?ë"˜˜r—á?µwÒۈÝ?Ç$¦Aª='?Å=œökœ?ƒÃíZlèÐ?–|¤Xªb?éçƺ+¼ø?Ånú;Sب?Ýr¨P°éÜ?³àj·íž	?¡:•™7G?‰Ë{®§?à6X.M÷ž?²ì~lÃn?ЈÌ–;?±Œ[²³Q?r8ðá.E ?n<À^ýÖ?ç—(ò"×?±Ãáø|`4FGL J1405.9-1853?íêrÂË@DHFà!qÀ;!¦Mà^À<\m¿ <@ Ťö!d?ü;cž5	Í?Ô-ÁÚ*ƒ?Å(ŒDâ?ì%Õ²NœE@êŒÒ‹Óˆ¿â*"Q€ü¿í#¸Œíº¿À'\HÖ2§¿çKýî,￟‹råOпïÿþÞ÷UNASNone?ï•äöÌs¶?‡ªÔ&E³Í?B‰¶$'Œ?<œJ'?‰e™±€Éš?‡7ÙRwÉN?ïOWU_>3?—"´P⮶?NÒGT'ç?a'ŒàÝ µ?•ƒs°£?–½ëcEKÜ?킪!ã€à?™BllÁ
?uJ]>¨?iX'
Éâ?²™ÊK?˜f®?²5?Ò–ì?'ýÁŸˆ:?Bâ`N¤:'?A[†%·"?§(É\ì`?'ù:»¯æd4FGL J1406.2-7500?ïïÚÏç+À)²<êlÀ:§‰i ­ŠÀ<ÖüÑwV@Ðҕäƒ@¾6œt?m?ÈG<)¦íj?¢'­€™l?×VŽ®˜.?ûµ¯¬ÖbM?êŠÍÿ&ç ¿ééH-–;¿àHe)O"£¿ë›—jë0e¿â!iÂ;yS¿ïÿôa¼2¡UNASNone?ï[L'CT²?"ÕðûÁB?V¬q¾q?WD+•>ÿÆ?"+¦Æy‰#?'‹c‰ÈD?ë4iNͺ?ÃüT/OÃ
?qQeŸ¦˜º?~ë7¬ÔŸ?¤û-ǔT?ÃÉd}Ê}Œ?쿁ùv5? éhäð¨'?"ΨQ€?'ÔÃûX‰)?º¿üŠ9ü?ž/Îp…O?ëñhc?ž²£	|?‰{¹®~a¡?yÏbñ"P?½EE®2O?s8‰u4FGL J1407.4-0820?ïùI‡L@IÄ"`À:¹Š '§À;¶@­o9t@¦óˆs@W£TY?ÌYAºµs¿£ö傮Ï?̎EèíiÐ?ý 'ç´¿ÔîYyîÙg¿æÄe©¿á€C‡>MC¿î*Ò§a)? ^vÔሿãHû"±UNASNone?ï6!ä¹/?Ÿ×sÁ­ô?eq.&f™ç?j6Á˜AY?–¤
Ie?Ÿ'?]Ï?îúAqf‰?¯|ìü?ãð#Ÿ˜Ù?"{"Õx?ªÓÝäu¤D?©¿4Ñó±f?çþ/­¬½5?¬W‹ûb?•?¥ÕF]gÖ?"
ö+2@?Êŋ÷µ±5?©cÊv|_€?êÄá6Ô?²h_óÄ53?i9;göÉ?ijLÏ
f?Ç4‹¸Ó?²JàZ—¬4FGL J1407.7-3017?»°5R•@=ÂNY)gÀ:Á°\S½íÀ<"(LOcë@¾t@ꗃ>äA?Îþhö¹…?ë©hyfk@W[_¢'@ûr'¦
?ÅRHw=#L¿Ó?š_<P"¿ãT5â:\¿ïhD¿ïÿÝƒ(i?îœtÀFV¦UNASNone?ßd‰^ÕÚh?Éob;`&Ï?×Ô³ëW˚?Èþ7ö}e™?Á…k¤³ü?»NX¹ÑÕD?ͼŸ???Èv,ÿρA?äÄXiÝ*?ÍfH—Pq?¾e¶z˜-?³Þ°©Þ|?ÖÙ®Á¦úú?°³Z>ô?ܦ¹Tc"b?³áϑ?Èÿ/ÓëJ?ªw‰]Å1^?н{dÉ[.?´O	Xœûž?âµKŒ÷Ë?ºiÒ"è­À?ïÛMjx?¬Ì¯®@Ã4FGL J1408.0+3834¿Þ´B"\@Q"-¶°`À;·¦ a4À=d2‹n@ ²->>T?ü̳¢Y[¼?ӚµUů?¾àŨ]_?î¤âè7Œ?ÿûR[Âsƒ¿ïږ";cƒ?ïõ·!iÝ¿çè§ô¦/ª¿Þ¯¦/OÏ?—øpƒd'À¿ïÿÒ³–šâUNASNone?ï˜yE©~?‹ù¸\'w½?KüI9¥Ã?JP©éD3?ˆ!ê
²-?‹HÊÐüõ=?ïz*ªÖÙ?ÁZôۅø?M	ÿÌ|Ó?`÷V~o"?£"ªø?Žs.´ad?íÎÅ´næ?"hI¡|G‡?uÇOÝ%î?døXœÝ–?°-™çŠüÝ?"¤9\í±Ã?îÓ
OùP?Šò.Î#"g?gæ
-ØÎX?eÈã"híô?¡PúdBÞ%?Š\æu94FGL J1408.1-6010¿ÏÿeF<?ô¾C·å´ûÀ9¹™	PášÀ:écyL8@ o+ˆÄà@õþÚf"?Ðli_À?¾"PTVC"?ò^FtŽ@–‰nÔ¿ïùJ¿@ó?îÄgÙ--`?Þ"ZÞGô`¿Þ8_~¿ïû ŠN¢û?ï˜l]vRÃUNASNone?ÃGså_Ã?¹6)¾@m¢?•v4RÉH?0(‰eƒ?ꂌ€p]Ï?»2H[t1?Ö]¾g݁?͈²ñÔb? xŠ²(?±DËhËC?ãêÏNóf?Íþ×ô×b]?ËVëuÖ?§®
%²à?¼5Ão\? U'u…1?壌Î7;ç?ªU¿Óðý?Ó»â4	º?»OйK.°?–+‡lìæ?'E?h~0?åp²ª"ò?¼®—Xf4FGL J1408.6-2917¿ÞWÑÃV¬_@> í_‹ÎÀ9¯»åüjÀ< ¬Ö(–@$ë,ß1@æ'öÀ?¶õIB¿X?¶[âÿ¿z?÷`ýV"U@]Î_ª¿ÐUýfȌ¿ævA:\ó ¿éÅ(~#qt¿ëp(¡ß¹9¿ã²€áü}¿ïí'ûî£UNASNone3FGL J1408.0-2924?ï%HÓ ? 2ÄÃ
ò›?ŸC4Z?|ç¦å˜Sð?'ǬûúqÁ?ŸMÖæØ-?íH¦¸¨¥U?´ØõF55?—Í5&ÆÊ;?¥®´T-þ¹?¯ŽùâE‹?©ñ¿FГ?ëՈ‡å?¢—æ5?¢‰¡šœ?¾<¢z*¿?»ü'î²€?o£ô.…¡?ìû
³fá?Ë=?§r"	Ô´?–UÌ2??¨Ý2ÅEu1?O!âXE4FGL J1408.7-3747?߃}{´^õ@6™Å£ãŸwÀ:˜³"&jÎÀ<`% Jù#@M"òiG@Os²Lï?Êz:°€?ÙqR=9œY@Wކ2´ˆ@$ð"ê¿ïÿû-2h2?ïÿÚÁ,/´¿Ý¢¿³Öh¿åø!ˆ¬6¿ð?ïý¡ñ&UNASNone3FGL J1409.2-3743?æ¡RùÐËî?ÃÔks$úk?½aГÐvï?¼x÷Jø?ÆÉËÎԔÑ?¿ÔBHS?åÁªJºv°?Ê¿.e	«à?ÉêýºØÝ?ǑåŠ=ÐÙ?¾²4|:¼?±ÝÜ Ý?Ýä¯,Hiª?³G¸[»è!?ÑßM]H
?² £Ü"Q?Ð<v›NH?«"aÏÀ^¥?陔PYXÆ?ªÓÜôFٔ?¶?y¦}?¡Ç3â}n†?¼óã×"#T?¢h?&	ói4FGL J1408.9-5845c?ÐàÛ
9œ@õöº «À9#¹À;íöé@Ê«V™m@Ìhĸ*?Í.rýMž?¬ÛMîöBg?ä£þwiÄ@$ˆJ'Ê?êy]ïŸ_¬¿ä)™A,5¿êI °N½¿éô›Gð¿á)zLÍ8¿Ø'Ü]¹oUNASNone ?Ççë/Å?¹`:'ùÆ?"J‰ôžT?~œ#©K¡±?éêО2¼?ºc}±ß³?Ü´ào7!?ÊÝo.è+?–QÏÔÎöF?£m9­0Îí?àóI½À=?ÊNT9žñ?ÑÖ2|<º~?¬ë¡\Eb¹?±NçÝ`"ù?"×X};?äë	Æ5'"?®ªAĂ%?܆l³¯·ô?±‰¥…Ù!?sŲ
*'?z)*WÅý?á>ú_û^?±(yŒŸë4FGL J1409.1-6121e¿Ýmî{ÚR-?Àû>û…À6›¾7ÔÀ9!zÈóú8@ «:ðn@(Ôº××Ã?›à¢í€L?¯¼Žç™@Ù¿Š¯?ø¨³‹™Q¿ïÐýH•›?ïðò`Û+¿Ý®êäâ¿âÊâ|azn¿âݹNjÇ¿ãA!"µUNASNone3FGL J1405.4-6119?'&®Ä'þ?¥d¡±{h–?\ÌHÀYÜ?s¦íóƒ'?ï¨ÿ!(Âr?¥¼}ß?†è¹NÐÂé?—w2×Pè?Û==KPy®?҂à/‰H?â¾u€?ÒCðÀv²Ó?³ÎI¸o?xòÕ¯d?´ Í҃¨X?œ]¹,îsL?ë'KæSæ?¥
ÈáÊi«?\Qäë\)?RB§å—Ç°?À‡´+Ö?±o"ÝàÂ?ë͵†'"Í?±'_Rà†'4FGL J1410.7+7405¿ìOj¸ýÚX@Dõ*™0¾À:[rðR
À<ojM{³Ö@ ú'WÛß?økŽXó·?Â_Tä³ÉF?Ñ
ƒÁkÔ@€Ò=Oè@ë3zQ¿ïÿïXz?ïþâ^.‰€¿ÒŽä;(u¿ºÅñ;lÌ¿â²€óZ€¿å"ãÓrÙUNASNone3FGL J1410.9+7406?íoN…mSP?«†xα‡?®¦*í£s)?¨+õ"¶Ñ?"ÉÙw¯ ?{¾±rç?îG­Llçg?§†ÛãfLÙ?‡­6;1?"6å~n	ô?¥™Çøcú¾?¡DP9Âð–?åGOEE?´6bë¬]?ÍD	¦vHT?²›Â§sé?»?:8êå5?ž£Öo¹«:?ë¡Z‰}?¢apw×e?¤÷HëþºV?'|áÿµ¶-?¼×Pµ´¦î? }´'"4FGL J1410.7-5945?Ǜ_nœã?ùx"«ËËEÀ9þAˆ`ŒÀ;(šrÝm.@ ¶é—îâ@ît¢iKô?Ç éD&Ëq?˜ÂsªO?ÔãÂwß5@¸áÜò¿ïé|Ñö®?ïól^MW¿çô´±M¿ÞêJa".Ô¿ì	íT+Ñ?¿»P¥	qˆUNASNone?ƌª/?º=¤è²C?ž Á¹q?ï?¯Ì°V?ékò­«p?¼¨üáéå‹?ÙOËÖTV?ʍE´Uä?Œ['mËóR?¤"™ÄIß?âæ«Ë¤ô?ÊcÒã[ÿ«?ÐrÝ?é?ª«ìH?µš)ìJb?˜›ZnC§?å¹L"ò¾?«¤g1 H?Ûc#î¬P?±ºpôõâ?–RX,!í=?ˆö;Xco?á›ÛGšo?±Ððóq;4FGL J1412.1-6631¿ï—ŽÜžž^À™V}»ÂÀ9ˆ̼À<Fí$[@'—îž®¬@UÒ°Y?¼€ìब.?Ùlæ³'à@*
4›èÿ@âd×-©?ä9pÏuôy¿ÓkŠ\å´$¿Ø'Äãõ2r¿â¥,¿ü"˿Wz:Y¿ïÿƒ}ùUUNASNone3FGL J1412.3-6635?YP0ûv¤?‰ßòEÓ)T?íú–æ=¨¤?¦ƒ6þàš?©=æ˜
?¢Ü–P'P?«ÐóՁž?©j°•ÕÏt?Û°ÿéJ
?ʟDh»L?àv>ðÎá?Ê&ØFæ<‹?£ÿ´™Üêå?'Mß›$?ëQù{?¤Î}-^Ñ?½
•ç8Éü?Ÿ9'Løü?Ïã{yYŸ?ôZ¸a̱?݋#:˜ü]?±1Öi)m?جëªVÓ?­1.ßâ-ð4FGL J1412.2-6018?ɔù"]?ð-}|,¡IÀ9δ#ˆ›EÀ:ég•:H@!1د8D@""úÎg×?ÆÕÿ{&¿ˆ¤ÒK«"Ü?Äñê¾zN¦?þ‰×Í0õÁ¿ïÿYø"'?ïþZxòZ%¿çÊ9¿¿H*¿åCÈü]´¿îä£î‡1¸?ç$¯!k4¬UNASNone?²#ÜU©?­^¢Ž¾Ð¨?ŽížŸ»O¦?—'hbA´?í?ÎV] ?°ÍSþfËñ?Å~/'ŸU?ÄQz#t…?˜›#t[¨I?¨1.kXÃ?éۛ$:è?ŀŽ¶ãä?ÈþÊùèH8?¦NfÒ
MÈ?¸âXxwx?›ÎJgoò¼?æ¤A6ß?©†PïãÇ?Ƨ·@ä?¬dè?l?˜oŽXËÊÎ?'y»¤×àT?é¸BãKÑq?® ò¸*ÜÊ4FGL J1415.2-5550?ífefÙuI@'÷na«À:—J4¹À;hoB­úz@^øÓeî@°;Ñgf?×nA§V?âÓïÖ½@¸®$kT@ÊÂOpU¨?ïë°½¢¿â#NžÉ"C¿ç9Á¢w8Ç¿ìŽÜajS0¿ç‰u"×'ù¿×WÝašy¾UNASNone?Ýk Õ!®¡?ħ3QP›8?Æ0K'Œy?Àþo'|?×|9¢Ê‹#?ÄâjÅɌ?П5Ö£'?ÂøCµD©¨?ÁØ=OÇZ?¾£*žÔÐ1?ã:V*"×æ?Äæ°÷Eë?Ö%ëú&]?¯q:çI|é?ÄÉbhs'€?«ïmRõ?ßubџáA?±¼ªo	ªË?ÒÅwÿÉ4u?«99cՍ?ÃY)«]-ñ?®¸ÊÃ%‡?áÆù•DJ?²o®Sÿ%Æ4FGL J1415.3-6110c?Ñå-ÃÔøã?°«ÝSÀ8¡=¼ùðòÀ9àÇÛÌD@ ÄÁ>ND\@ŽŒ:5…ô?÷™»È˜Š¦?ÄNž·Ëß?üG7|n¨@m |ŒÃr¿ë6qY´¿ï;	á€8?æëÂZƒ¿å®²šò_.¿î'lU"°L¿¨k¶B­àµUNASNone1? ;4ؤZ?§¥€¬±·¾?Òw?Mµ´h?Аë|"5t?åÀ¯uכ…?ÑÝé9¤?¶hˆ {ž?ÀN—""?±vQE¡?¾œYóÔW«?ë(Æ7Îj?Å
˜
ôö.?»C"+en? < ²¿{,?Çî÷0Ÿî?¯ºH0Y":?æœ	ÿkW?°xóú¸ìØ?­–_ù@á?¯ÿÈJ¢?r²(çrf=?"*IÀ'?î5½‡%?°ÿhº(p4FGL J1415.4-6458¿éŸø®R
À]±~'­À:"=n€À<Píè¦G'@®:»gʕ?ýlÇß'Bd?̛ŏÝ?áB!"9Å@Uþ9Vc@hZ‡`%?éHtxwàâ¿å©ÚúŒùx¿¶l=?üoR¿Ô /Jpfš¿êyþ(kB¿çy0m†XUNASNone?ÈG3#‡°?·úŒlž`8?Ά.ëÆÝ?À´øÃôÂ_?âL½ç|,\?ÁÔoo»¿)?ĒªÏnÞ:?¼Ö>Nß÷?§WüŸ¢ÇÇ?¬ÒC}ý¿p?éeՂ*ö?¾¹»á»Æ?ß pùBê?²†T™0V?Ϊò/µHü?±™Ó@å»?ъîã?˜?©¤ð.‡û?ÛÒ ðYÿ=?ªëg¨ìS?Ãˆ}?¨K»Ûíì?Ú6@áÁú?¬£ÓÌê´4FGL J1415.9-1504¿§(dM1Œ@EŠo½'=\À:ä§0ž-À<€ÇÛÌD@e¸Ž|Z?ûWÓ[\G)?ÙoDü‰Rú?×8
2ˆéH?øÜz9'Í@"ô7ŸÔq?ïå' Pˆ¿íAýa¿§Ë.€à©è¿ãÂÜôb=¿æä–bWŽ¿ïÿ´JõǘUNASNone?í£Š–ü'?ªúIÛ‹}?xÜ ßÍÉ?q'›‡?±Ué^Êð?ª=Îý˜?î. ™±,?¤O-¦ˆã4?yV¥01HD?2À·¨?©ë!ÉnÄ/?¢Á..©?ëfŸ¯AÔ?¤Dè
«¤?žÐH,"3?‹ŠEÌ*}ø?½ŽpzèÍ? Û§°1=?ëxYŸÑªÃ?¢êą6?ÐDEŒ?x10?¤n?Á•<`"?¡f—s0Þ4FGL J1416.7-5023¿ç|õÎ5@$mG8£µÀ9혮¸ÐÀ;øÂ!xÌ@ð·S=êœ@)†@÷A?À$œ—zÛh?Ӆ2ˆJ½@Ø.D¶é6?ø[‡`ﯿÒ8Àr×
¿Ú¬ìݎf
¿Ýê1!5.á¿æ
ÌÁå>¿î`ÊE3¿ïÿÿ&¦³UNASNone2FGL J1417.7-5028?±7P»/?§
¦ÓÚT?ÑÆ]9°¹‰?Äsű¢?äõçKÄ U?ÅNo–G¬n?ÇÊŒ†#?ÃXüšhi…?âIBž·Õ?ʐ`OK?ÏÖý\š‹?Å[ÎzU4?Ê=ÑúPШ?«\þ5Z?߆ârH—?´kü˜Ó'M?ÓZ4åeO?¬%Ã+˜¸/?Ëm€ŸòV?¢ïr«Ѐ?Õk.µZ?±¿'ÝΔ?Ý-Íû|?±ö8b
Ü#4FGL J1417.7-6057?âñòSDÀ?ÆÊ#åbÿÀ9
>¼(À:G¨=¡K?@$x‰1l‰–?ý
¾4ƒ•K?Á…NÉf»Ì¿©ÂGBÒ/?÷€.>ì?ýîé':,¿‹?à<Û?îf^ê–¿î虱íM¿à³-ߌB¿äÊÜgtƒ`¿Ü'-ê
ËUNASNone?{·8©cT?€ÐpÈG–?[UŒŒã¿?e( <hv?ï¼CËGæÇ?ƒ»tD4"ñ?œ Ååg±??«v¿Ò1Úð?£ü)*á=3?³+bz!©?íß7>&®£?·vÿòS?Àn-Kǚ?¡…3JJ?¬?s*˜Ù²?"ïÔKû…?ê ˆB€?¤"¦¡à2b?vDš4p~?lZڄËx?™¤›ì"™ã?œ×¾"ž/ú?ïQì3BP?Âjýñ²Ê4FGL J1418.2-5400?ÏòLŸQ%@áÐÈ0À9ýH"Ô·À;}±CÝ¥@Š0NÒK@i"/?ÒzJHùn?܋AèÜy@èí¢/jQ?ø;O1¡¨?ÕÔ3~1´-¿ß{{áͺ޿è•.enâ¿ëOñå‹	´¿ïûÎ!á|1¿ðUNASNone?àNK¶ ÷?Æ6•Ž^?À5B^:f?·u­
¼Ö?×Hǎ± ß?Æl÷d3F?¸,U–w7?¶è]ûo?Öç_¹'Ã?ÉÈW@ð·Ð?á†Åp©7?ÆÏ("R³ž?Ñg_ØB\?ªÁ[~d?Ç®%'
Ë?§\Öÿ‰oL?á`ƯN?¯w"ûÝÆ?ªTC
ï5?‰D–íôù??Úðmêû3?¶œ…Ôû?àâ¹^Gs?µûΣ;¿4FGL J1418.7-6110?ãÿ[[àl¿±†SÁžˆÀ8!å±  œÀ9Fì\tu@ör~!Ãõ@¢¦¾EJ?àì){D?ÒXÉûa4Î@
% 8ð?øìWÿÆIP¿ïŒœ[ú?çÃEš>H¿è&@©-¿êcv'-"Ž¿í!­>¼ÿ$¿Ì‡´÷UNASNone?Œ¬‹×Òy?¡qçš_%™?¡€ì?²Ï¥‹Íþ?î}?iÏáõ?¶Ér4"½~?'G£ì'Ï?™Âc~?ÈÜY=A?ÇàB2‹r?é6±#8$?LJ×i®«?³4\ÞÂ?'êXCŽÅC?ʺù–#'?¯0Ïyf€?æêüÖ»H?°Z¥/Œ†?UÖ]q]à?FÞ¿¶¸Ö?›·…†?j/?™Ý—qoî!?ïX¥EËÿ?™çÐKŠW4FGL J1419.2-6029?ê´¼µ¨n?áöAÛl¢ÁÀ9"›vékiÀ:è‰ÁµB@!"|¨òýä@埱áŽü?سÑÞÚkq?'6¶ e©?ËÈWÈþµ?ü®¨Q˜N¿ïÒÒ4ëš?ïŸÄ UàÝ¿èçˆ9õÅ¿ä"ABÀnð¿å?¼xÁ²½¿íÜ¢ÞìâUNASNone?¶"H/ ?‹œøÍ\Ù?æè¦j?Ž-"ܨ?ï2°8üs?—IñùQi¼?°yÜ[Wùú?³ä)zð´K?š€ã¹€B?©Wß«Å|¹?í½VÌ¿?¸Rðœ/%Ã?¿œszû¶? Ž1D‰-?µs:ø9rj?žÝ+%'?é^
1™n;?§<Ù¸|L*?ž¾£Ïy?‰åO˜¿L?|®žcÍt?y–¾¥5?îв†œ?ŽI5‹?˜¸4FGL J1420.7-6701¿ìLÜ)a"ZÀ¡©É'†À:ùp™ÆÀ;™oJ:¶µ@=1¦ì@^]×M?ÍmíCdٞ?Μ
!Áñ§@a&Ö.?ùyÕú
¿ì@r`ð…º¿Â¶YÃÀ´'¿çtè?ƒ¿ç ÄÍ¿ëY^@'7|¿ïâ[>ê÷ZUNASNone?ÁaiÞޖî?¶˜œŸY? 6ÿÞ?¨Ÿæ Á£´?ê§"&gšF?ºüdÁÅ?É0WêÅZ^?¿h™BæÂï?¡£ý9¬t?¤Æ',R?虪1³â'?ÀÒu
Ck?Õh‡C?°-¾T"W?ºìóg$ƒ?—ËŒeà.†?â-OŠ
Ï?¯Îºâßd²?ш Z>Ž¨?©^¯g@W°?»7'sv? Rv¦+"?ãÔ¿'rU^?­]½	r¢—4FGL J1420.9-6127c?烈^™úy¿Û T¾ôÀ9pAK#êÁÀ:oê–â/5@"Ž™¶Iþ@ð®Ý*?ÍÄn&NH?ªü8ö?è=Pù׳@{…UE¿ïÜ*7áï|¤ËüÃ5?ïø4SÅz¿æn'ûnj¿çnû€"dü¿Úÿr;†¾ÌUNASNone0?¥¶þ‡Ž£Š?¦7h-Q?ƒ=‰ör?"DÕÒJ¡?îW›¥bÁî?©óÚóG¤ä?»‹V—\?ÀRÞfì	°?‡Ôrûœú?¤†æcÝ?ì/Ca3•?ÀÛ=,·û-?Ä@äœ>?£)0'?³Fh)^bö?›Y)[ó"?è‡/vÛ'?¦ vG9ú^?­ÖÕ==üÒ?ŸùåÊ°?sówé/?vÔ'²Iû¶?íú¬<N"? Ÿ}ÈÚ4FGL J1420.9-2431?ã¥"LðÁ@A¡ýiõÀ:^ÏO^%À<dëÄØí@çÒøŠì@ƞ<–‰D?ŁÂ7rˆ?È'øR¸@_Ô{í·?ùˆ¤~Ïê¿Ô²ŸÅ,Å[¿ág—ô}뾿ݓœº¶¿æ¸]¿xÑM¿äV›†Ù£¿ïô›]i¼UNASNone3FGL J1421.0-2431?êÅËÖ,Í?¸-¥'Ftô?–f¶ÕÂr?'
Um€…¼?ÄÈõîþŒ?·?ëÆ93‡?ëð"c¾?³‰÷HU•?£?ã#?¤3ÝÈúOÊ?¶ôCDð~`?ªϘB°Î?ëɺëø)?¡mx5^»?¡°¨x´ü?Ü†$H o?¹%ÐRËä=?™¦@óŽîÁ?è—]º–¡"?£îìã£.?²2@(?—y¢"L±?ĉ†u›eá?ŸÚ‰J¤h4FGL J1421.4-1655?Û&ï]ps†@Dj}¿H€À;'œ%eWÀ<¶´•žbV@"á]¶"|#?×2¼ë®9?âΈ>''ü?î0öã Ì(@vA……@f&ż:¿·Ø\wûT¿ï ˆ¡#і?ìIØá®a¿ïúÕ>
|±?ïöÞï@5¿ç.ÄÑ¢UNASNone?î}N{Ô0?¬%sxí!?z[å'eɘ?"/9³&ã?¤ß›UöË?ªVýÔa¡?ícÄð$ùy?º4Ôö}ý+?‹¯ë0!?¢a'íЛ?±kö!hN5?¶y»@U
?ê)RÈk;?¯åB«Î¼‡?¢{d€euŸ?¨O8=OÕ?»ÞÔÄõ¬?®Fpuju	?ç
•2|S?Ä-Bß0Õ?+ê$
žÏ?@™çiZÎ$?ÑçXWuSš?Ä-–¨õ°A4FGL J1422.3-6059?í0Vi:£Œ¿¤Âþ*Æ[À8 6®è¶7À9­O©‹%@ FI²ül"@¢Ä?ò¥K´3xÓ?Ír‰Ië0@ƒðØï?þXËÁ	8?ï| ï
ê¿çú(»
,ª¿ã¼²F+]¿èëë†Ì7¿ìñ"b"4¿×r9Ù?¡ÖUNASNone?•_Jé]ͤ?£@Bäù~?ƪÆçÄ`+?ʝä¹lŠ#?éªSîÃùˆ?Ì
(@µ+? nbëÆ?§˜P"ùˆ´?±  ˪?¸(	à*t?ìÕjoJ)?¹NB@&f:?´8cœ)í|?–o7Mh ?Ë ²±CÈ^?°d+êâא?æ°Æà)Ð8?°ãŸÛiU©?v2vÚø§e?sJ¿\-O?~.÷T	Á? -®ë+?ï—?[f?'}I•í4FGL J1424.8-6536¿Ê‹4"§ßzÀâ[úҙ•À:&.gòXÀ;€å¯º@´ºÃ{@ÀLÁy²t?Ù>Nî÷ð?é2užÎ_@p׈§@&{Ÿ^?º,×#'×?ïè¹\­€¿ëÔ.béÚ¿çÏÚ¾|ýؿؓ²Ï˄οåÛíÎmUNASNone?ÊèFúò;?¿ªø°H…Ö?Ì?"<Èþ?ĞJ>½Y¹?â6	ô>à?ÉETsgD?ĊSÖZ6~?ÂåUÿ–€­?Áô¡A!f?Âà¹-(?æ}mâ*?É8ÉԀý=?ÒVÇMCÇ?©Æ¤±èD?Å>ïY.DË?¨§æðe¤?á"্Ìé?®mÑOódÓ?njû{@#?´W…à¾ü?Þ
9«tß?Æqè"Þ{?Ö7£È–ë?Â:wÓwµ4FGL J1424.8-8012?ärÎa!ƒÀ2Q֌i/À;¤š~›çÀ=IÄòø6@Fé—îâ?ÿé={‹'™?ÕªÜ3?ïÿ踻Ð@m$
<ÿ?ý^g×®6¿ç{½ ´ëÛ¿êá|¢¿·†ƒ'F>(¿Ù‰ÿöÅÅ¿ïþ¢½"°S¿íQ&ΠâcUNASNone?ã?Zb\;?É9ŽŠÇ˜Â?ÕË$Ës·3?Ȧ.Š0¦}?­­þ<'¾?§^à';Ûï?ÒC‹]"*m?͒6Ç2Qã?â}ðoý2?ÐËô¥æ¬?Á'"ââÌ?»—
U_O?Ö·R'F^‹?µ¦ïÖÑ،?݁¥d=«Ò?¶BD2'ã?ǎ÷ëD?§™µt€Óì?ÉÞ jŠ£ò?µ‹Šùåéð?å§hÈßœ?½õ–oWW»?¿xãì‹?±‡KzÃfà4FGL J1427.8-6051?ïBò\ÿÂæNh˜Å´À7™ʬaÀ9æ?Pwç˜@,ÚÏÄÎÒ@ùü£T-?´õæ °Ï–?ÅÅxDµ;·@9	ۂr?øÅqœ+?À)nä9P?×´ÿüz¿çÚcŽDÑÁ¿êÊ*ü-©¿åŠØ5¶›2¿à¨<_+߂UNASNone2FGL J1427.6-6048c?©HZÁÛÁì?¦î^=—Š?²ãI¡Vö?´Dž,x?ì2n?ºÖmˆ"°?ŒÝ¸ýƪ?'ðÚFVú?ÜnZIªuP?ÊfY¯"7Œ?áV[dFÎ=?Éó¬Î†f?²~ T#¥ ?˜¬Ä_ÄìÁ?Àd¼­ˆV‡?§%gï7eë?é–üÊuª?ªŸ¿|:(C?u,ÊÃoš?`Ÿ&ûTQ?ԚC´í1?³ç2À•À"?刄pˆ?³Ýsý¶¢4FGL J1429.8-0739?…bþȊ'V@Gìd^NiðÀ;fBÀ<ýÔ£Zã@X6hqÙa@UinX£/?Ô'Ӄ 3?ì|p(‡Ç@[bâMg'@Á*WA…[?íħÈ0†?ïó'?	*K¿Û&ÕøÎ]¿ä՛=ÈK¿íö9ãPœÑ¿ïÁPb#UNASNone?ʽ‡B?¿«£É+Ã?ä½x«Ò?ÇÆVð@îœ?ÅîÉx?½Ô
#a$°?Ê}l¥^Q¶?DŽ´K!Nù?呢N†VÛ?ÌÚnkë=è?¾xA¥º?µV/'é#{?ÞÝ	ðZw?µˆhdØ]I?Ô°@ñ;!¼?¶³±Uè?ÊkÄ	©š?¦—
¯/?Àåå¯?«¬hOˆýR?éûCå¬R?²|ƒŠm—?¬¸Çª~?žq›ê¡ä4FGL J1431.0-4432?êüjÊhˆ@-Ê¯¼ÎÀ:Zy¯ïFtÀ<"¢"=_@ˆ´™û@À#Uož?Òø®6Ý?ÄïäêOêy?òåQÉ oâ@ÉÎÖ俾šP£±uƒ¿éÔÎX¾7¿ä+¢zé«*¿×")ÛE¶n¿ëQ(¡´Æ¿ïñwÁØ}UNASNone3FGL J1430.8-4434?ìÚݹ޹S?´úgý?ŽB?oÝ#,‡lš?g~ğ!ZC?¸*)¥ú?´Á½Ñyâ?ïŽ9ühá?4RR‰'?I+e%|?Zò6TÔ™?Ž‹ŽÊ"o®?Œ:NÌ›?í*#aÏd?œÂ":‹º?‰9Q⾎«?B43¨R?³‡½ ™³?™·Cì(ýK?ÁÔ¯ó?†ÔÕqƒ?hÿG»o~_?[D'xÝû|?¦fÏfþî?†n-Ÿåïñ4FGL J1431.5-6627?¾h"x~}À	‡Æ2~ØÀ:CÇE¤NÿÀ;±•ìeïH@äjÔ4J5@—dj㣩?Ï_T¹À«?Ì!^IŒf@BÌÛæED?öAkBS^?í:1…ý¿à¾Ý®‡¿èDƒBL"¿å"M!pèö¿ïÿò> w?å6YX`êUNASNone?ߐªµv?Á?à‰s?•q¥›±?lڔ[5?ß:òp-?‹p###I?ÐÅËZëY?Ƃ[@
ʙ? .}A´ªï?¦'°tD?æš2~oÏ?ÆцuáßÒ?à\fŸö%‰?¯ԀhŸ?µè·c¦?™k7¸t¨?ÙÍçS±D?¬ðËÅc ­?Ö;PÆóèX?±ÌTÀh?·;®*ðs¦?žþ	ýù/3?áúá×'ý_?±én‹Z4FGL J1433.8-6357?îÉÐ"}6À
R˜˜—;À:áÍ:°ÕöÀ<§³Ó׃	@GpxŽ@¸îÿ&¼,?Ö×.Û4ă?ïÿ—?LF*@
φþŒby@6Ö)—Óò?îª÷?g?ïä;û…G?°1æA'òa¿çx!m
¿íñ܆~3ã¿ïÿ\‹/ôUNASNone?×ïï'©Ô?ÆyÞ3ÈhØ?Ðò+ÐcB?›†¬\&=?×ûåòé?Æ­pd‡R?°g@Œ¹–V?³*!ù"²?ÖNú¯ùØ?χF¥'?âåpqÐI?γ¯s±qè?ÞÔÔÁî©ì?±}#Èh±?ξ/í7Ö?¯H¬ŒØüù?ÑÌG‡:)?©&;'JM@?À§ü³.#?®áñ¡
l?é:­¹Kã?·ÅßTg"?¶˜ÏD¤?¨ž¬ÓŒ>A4FGL J1436.4+3900?àèV$¤Ð@PG͉‹.À;¥á¨&$WÀ<ë]à…ç5@ `¾$ƒæ?ÿÓ¯tÍ1w?ÎÆCÜ"Ö?¡SÀúå?Ӟ¤Zè®Ö@3Ý	°Øпëkô0õk?ä(½ž†"X¿Ü³T€µÇø¿å†žEÑ¿Õ½ÄܓiT¿Ó±<MŽ(LUNASNone?îïƒ)&»M?šÑË~åÁ?`¬×ä¯Z?YIçòÛ,y? ¢ <?™V´O@Ö ?ïwœpa¨š?Ž¤¡Ëið?H‹
ôSÓ?YZ¯.ó©?Hœ(T?CP<vEh?íÒ'¤ïÀ\?"A+n¿?~ü§Û"Àõ?qŒs
¤r?®ý𵟢?'¨øôJN?ï¸Å/Q?ƒT*œ y?fÓʌm2?_ k6ž‰?™.n(,?ƒ6Ô)lü‡4FGL J1438.0+0219?ÀJó@;ã@K6-œñ<ïÀ;MÆF ÎAÀ<¦MÝÙe@4œ´V3h@Y¨Íê>?Ñö«XþÒ?ŊnÙQ•t?ïXBKÔê¨@¤–^PÃ<¿íN¶È¥ ?ï÷䨋¤ä¿ç‡âg^3¿áv"@Áç¿ä©Y?·P¿ïڅAÈÍ9UNASNone?ï¨m8€½?€ÆgÈdû3?Su/[?Pôä¶R‰"?ƒÑ
ùåX?t dR?=æÁª?‡½Š/S5	?FJ@ñG}?V±w¸òy#?‰,O"@?†O¡Á"Ü?îZÀ&*?Œ¼ƒ¤ŽL@?sÚÙö¸?g[["	?£¯ü ;?ŠjkJ4(?ïeÄÃ{?wiB›€?gÃÆÛLgÇ?WÌ7eKu'?OƒÞ®?vAÏF4FGL J1439.2-5142?ߤú©\Ó@ºø>jžÚÀ:"…fîÀ;¬ÿðÇô@ìüÝ5М@®}Vlô?ÐsÀA#6?È
‰Æ½¿?úRš×‡;?ýàwÇaÓÛ?¡g"@
ƒ™¿ç<ž_æð¿ã«4–àµ¿è«e©¨–¿ïÿúVrÓ\?Ó_o|9·\UNASNone?Ԅ!8?ÁyÛN÷†}?"¥ÖÕG3?Ž1+´ÃÖ?åÀƙ¹Á?ÁìfÄÃÿl?ݞ¶ŸêUÉ?ÊÊVòÔå?¥ûÅ_ÚIx?§à6ý='?ߡдa?ÊÃ1ûä[?àĦ^C^?¯"
û¥š?·y#á*Ó?šj‰ÄÀ—?ض"úý.?¬Üò‹Å,?âßëˆ??°Ä0ns?¥
{ÆE¸??'g"`ÔÊJ?× r°&Êç?°»i
Å4FGL J1441.4-1934¿ê" ½""@B¦µ(À:ñ"Nü½À<{Ó"Qc @!-"Pª<?õdãåFn?Õ3_¿-R?à
¨š¾\È@"•ƒŠcœ?ôùkjÏ?½|­_I<¿ç9äàõ?ؕAED­¯?°O\8û¿ÇRl´^@þ¿ïýʀÂ2?UNASNone?êYo'»!?¾~ɵ¾Å?­ŠÑq…\L?«	¸ô­û?Àoå哼h?¹cì&{?ë*…Îð?¿ê3y"ã?¬&$‡1tD?µ8'&
Ü;?¸˜ÄÝïÅÇ?±æÛoþw‹?é«‹o¥?¨õÈîNys?¬¨ÈL v?˜ý¥Ø`¶+?Â)ƒ¿CiO?¤j60W?ßôjo˜`?¹kñ UÛ:?Á½>y–?—WՕK³?Þ/z"¬€?ºþYr0hc4FGL J1442.0+0732?Ñ0vY<v@L£ä`gHäÀ:݃¡àøÀ<o?v7"Â@2G?ڋ|@aÓÅ'j?Ð1¾"ùò?ÕGfÿ1?ÿ0	}WC´?ûQ0αÿ?ï¦ÿ]ꏿã°É–·g
¿á™î=µÃ¿ã–€À.Ù²¿ê_`—Ì:¿ïƽ FUNASNone?ã&ÜêÒ8j?¤ãA0ÎÑ?§n¶×? 7ÇáY"?ÖÀ"<"ÍP?°'F=ü!?éQ©àTñ&?¿Ä±w¸È?¶ttƒ©ý?·2ÀÆ\Þ?¾þ<üÔÌÓ?±çÐ,¬t?è¸&N…î?©8RŸÏé?³?€'½·-?™SI"×J?ç†ç²?£J+ø$2?âOßìTo?§çm äæ?ņ=Z¥HS?¥Êm©»7n?Н!z}Ì?¥ª°£iZË4FGL J1442.1-2800¿âs'ó@<ÌRş±âÀ:|غ@ÙÀ<A˜ý'gv@éN
'@cq|D=?Ƒf"ÄJr?×âûã:Í[@¶ˆ7q†U?öKÐc\0?ß¡—_,¶A¿Ýœ"`IÁÀ¿æ¤ªÚ3½¿î»CÝOÒ¿ïù~¿\¢¿îvª¡~ÀOUNASNone?ã3Äñj?ÊW[XÚiŸ?½œûí4»®?ºhò´õÔþ?Ò17"vÊ??ƨ‹u°Cú?Ö¹:L©ÙN?Ïxώ)¹'?ßÑt~Õ?ч'žo5§?Âê¢i1¼?¶·MMs?á.
|òj?±—ïBæ?É{"ύY?ª(œ/Ûý?Ñ&êžT~?«u(¥zà?ÊG1@7Õ?¤ŒBÿ«-?ÞýÇjñP?´Ãà%î%>?ÓޟôòÅm?°AÌUî!¥4FGL J1442.1-3707?ìxþS­|%@4­3;–¯À:ÏeóSIÀ<"­Ù©T@ 6šn*Õí?þ'Xœ‰8?ȁ'ºýíV?ÁmhxºPô?ù¿ë¨Z&½@\"H?ïëy@×æ¿âúò¿Ðû¿à¥lZþ¿×i#°q¿à™RÓº}¿æ±·û"pUNASNone?ïó ™m2?'Ò-ÅIô?h&rôR…Ð?eúpA
d?œ͎H	
?'zâ]p"?îjî×¼ƒ?¡J¯¤ãÙ_?tcbŽÌK/?|
P6)Âw?¦Ê"Àª®d? 8pÒpê?íãx!¼Ñ?'Ìi¨•?wþ˜™Ó;?f¿ÍeÕÃ×?®Èº'´=?'o¯øˆ;?ëáªÓ"š?—ç?^€ö?")þ7T'±?}
`¥ç˜2?¼()ÚƄ?–ÿŽƒ4FGL J1443.7-7037¿àUÓ):êjÀ#‡ãÑÌÀ:
j»_¼ÿÀ<¸{0œ@rôf¹@ó¢#«×?ÁDyA_ò?À?PøÀñw?ýò–³5L@ÙÌ¥	º>?ïáö?6÷Ž¿âÅõåÊË¿ä_²?¿à²üÁ‡¿è½/Á
ÑпïÿüoQÇsUNASNone3FGL J1444.0-7033?éåÌ#jhu?¶#ù¬þe?˜8bp?'¾PêØ?Åa¿ê+?´˜°ëžd?ä	Æø—‰?Éßþ­€›?"Ëݲ›cG?'­ÜHÇ)?×Go"yõÕ?ɏ7Ì`·z?ê2*•æ†#?¨)ƒuâÃT?˜xå?49v?…
JÑɟ?Ä(9`H?¥uòFÍB?éw¿û??˜ûÒñrq1?¤ìSœY0õ?'}u/h?Äåë+íu¿?—NÆüâ"Ï4FGL J1444.1+7601?È» ày—@C˜P%"õÀ;›Ãèø|~À<÷Â,_Ú@QRÖç'Ü@E]Ø"k?ÔZ^ï®?ËC扷N`?ï>~jê?þÅúˍ³¿î¨f»ö»´?ïüKuIX9¿ÔD­®úSï¿äÏBrì1¿ã1ÿ÷œ"0¿ïý³¥ÝuUNASNone?ïP˜k]ô?' 9^û?p5U¢D"?jœ¯˜«‰S?'ߪJÃ?Kšƒsc?ï1¶]§!î?•6Z'¹<"?_*þ'úŸw?jûvlÔCŸ?—Ö"hœN?"[‰|88¦?í@€È.7?™ûƒŠƒ*Ä?"?ƒDÈÐÁ?‡$"Ưԃ?°ìŒZ?"Ã_Üt§?îÕÆô/ض?"ù²LX1l?è¦Sc+(?q••¤67?L÷å,W?'9OÉ×4FGL J1444.8+3645?ä‹;¿…@P
·AJM+À;	5œ™ÿÀ<r@žUÀý@xi^hk#?üŠÉ‡î"?ä!j³Ó?è)¬¡´N@8³¥´Z@͓´RW'?ïh<>õ‰/¿éHQ¨i@5¿á¼ˆ¿îm¿íQ‡aˆ±¿ïí•Ïà}"¿ïøtP3ôúUNASNone?ëÛöQ­?»×ˆôTm†?†ñ]78(Å?‹Ú.{ÅìÂ?¾IŒ¦‹Žn?»Ohjvѱ?èËCî"ñ?Æ>Ù¶ôcô?¹ùßÅ|j?À'ÃݗöF?¿¬Åë?¹S›0¡Ž?è–Ú «ã?©š¸n€:?²HF—\C¥?—&%Å+oæ?Āt3ß.ž?¤{/A"¸7?ä's0¶Ë{?¹ŸdÙvƒ?­W)JK£i?¯‡^Ûag~?ÓP4uHô ?·Ú{v¿‡ú4FGL J1444.9-5939¿ìTۓRò?½Hô‹(À7à°.0"óÀ9Õ~;oA×@ס–¾@»œ=¸È3?»ZÀ?ö?×)±>y@ Vlô!?÷ɋúŸ™?î]/Ÿ¾w¿ÎIÊäÀ3Œ¿æä:og—¿ë^u×±ç¿ïÏk¾Td¿ï÷ú"‡UNASNone?ž»g–λ?±†lNÎa?å ÕPõ;?ËR#j'(?ÒÔ	~䨞?ÊD"y>?x÷ŸÜûÏ?ƒËƒ;rß@?ák—næ¬?ÍœpÁƦ?ÜÄò¤~Cj?Ìø'š:ª§?¦¤3a?•qnlҀí?Üá¿Ø‹'0?ºÀ6ҚL?à$Üݪ†?º†"ý"*?%ò¥Ñá=?»®ê€y?Þö'1æ?µÙT¹û"?àõ%¿Ó?µ§'ßé4FGL J1447.4-5757¿ëj(1™Íh?ø^Ç»ëÓùÀ8‡¾[ðÁŸÀ:¼ÏJ«@j33fà@ký."h?·R‹íš<?ÜVômû†@û*ÂKi‹?ú"ŠÑ¹õ?ïõÄ"`¿ÓÏ© Z8¿æMOÿqº­¿ìzÆ:"‰¿ì¨õŒßvó¿ïþp]áÁUNASNone3FGL J1447.3-5800?‡ùÎ÷0±+?'Œ !a½?êf®dË?ÀBüiq?Äè@Vü©Á?¿î6y¯¢?"Šõk	B?'ɕ®OÀ?àäOé¢Íl?Ðó'íºp,?ݗÕß?Ð×æúæ-»?©_\8=ò?—~-j9?æ¬(§š¼?´Rì½Q`'?Ф¼,©ÂÉ?±ëK{SՀ?[Ú¼µR+Õ?E›ÊÌÊ|?ã­(µ^L?´ŠÀÚ°o?؉îñßñ;?´" ÓÁ"4FGL J1449.8-5923c¿ï[U æ?·a» ™VíÀ8¨f±åÀºÀ:B†Î»ºV@¥{Ð'@jTà,%"?Á¾x÷¼Q?×Xö;[á@•!4y@¦ã™—ì¿Ý'ހÔPп£TcÀªæ¯¿ÜßLÁ¤¥'¿éFÝÕ2ÌÜ¿íÏr™{¿ïþ€£ÿN)UNASNone$?"‡S	@?ŠgF{JÉ4?Ä%Š¢£ì?½1í²K
À?êZ‡
¿
?¾-˜ŽûŒ
?–Î~7¡?–•ó;j¨­?·œƒ6øÐT?²Îž¾Í°Ò?ìUÿ
/-Q?´Š"\?«³ˆš…‹?<œ,Q…?Óé³ÖŠß¹?µ*ésQ?äOí'ÀçË?µ.ü«W´?…9oÎ<?r&X¦Åæ?¸¥û†FNÄ?¢©=AÛÑ?ì—©wý7?£m¯É5A4FGL J1450.8-1424¿ã3Ô7œ›Ï@C®Ûʖ'À:ñ9>/HÀ<«©Ìíƒü@¦o;÷ýÓ?ÿ	‡ƒ U?ËzÆ[¯S?àšIÂÁ±@b.ä¬?ýZæØñ~?ïÿ•!îZ¿ß°nh@†¿Ðä¶Î]Ç¿àd"‰—Ã׿ïÿþó…õ¿í<¢¤@UNASNone?ê	g]³9?¼wÐG9Š?½|:ÄԚ…?·íÚ´Œ"q?²8ŠM'?©'šSlR—?ÙÒ¢'¥£)?ËBAr
ªÆ?ÛôtAßé–?Î]g…¨Ö?ÄqÒVôæƒ?µi{À§¬Í?àù幩_¶?´¯v-Œ?Ò:.xÓ?´ªÒø.õ?Ǥ'´Zü?¥«4›Qqª?Ónù:'|d?«Þáû4Û?ÛÝ©['Ÿá?´k\¥>?г]jFã»?ªð—¶¾ž4FGL J1451.6-3726?ÙäԊAþ@3‰ ÝDÀ:†\ø(›*À<*ÐíýZ@Ÿ¹"uö§@ž¢ûB+?ΏbÞòi?Ø}VÂÚZª@'!ý€É¿@~AÉùÞ©?î¼´áɉ ?ëmô?,­¿ÚLǤùv¿è<¦ÿ³©æ¿á+þöë"H¿ðUNASNone?è'LñÏ%;?½©·3Cœ?ÀÕç_¸Ç?¹	F#ýD?¹ÁɲИ?­a\Ûe?æ/d¿r©´?ƙNľƒÎ?Æ!ïûå?Ä-É1{w?Á$K9t?´E73¤*ï?æ¦d§.CJ?®ÉZÍøR`?»©ÔN9?¡3ŸèŒ?ÇÖ¦Ž\˼?¥Ír·Ñ\?á1Î`2‰?²n'í
?Ëø¥s!°?´Y‰É%%?Ï@!5Ð'?°ßÃ6Ì¡4FGL J1452.0-4148?㳘àOû/@/J^±¬À;$üȼÀ<ƒ|Æúû´@ Êì=ÖOX?ÿ´W£U?Çú–È¿\…;T%Ï?™ÿÑån@T$Ñp |?¾=‰ÎJ{N¿áû¶úÓpU¿Ú׶_Íðä¿ÜsÿÁ–¸¿¿Ý<ñ¢ðŠ¿ðUNASNone?ï­ª"ç?'µ+ûÚLÚ?EÞrë~Ë?Bßj´À?ƒ7•Éí}þ?'P³'>SI?íÔÕ*©'å?´j;Júd?_"©{?láՀ­ˆÛ?°ÜΞP¸?´5!Ž=
€?íƇàª?•1¥Vd<?x#ÞÝð?i+vÖZޝ?°J.ɱ±7?"Á9#ä6?ìÖ¸€7`–?—
-±bt?v§/é2
D?f†¶ W½?·ßÈÿ±Ú"?—bqޙF4FGL J1454.3-5551?å½Åo$>è@äI:ÜtàÀ9ö¢ñ10$À;Xù"«ô@"£ÊŸöÖ@zh˜q?ф}*[?Þ|´†"éß@Œûü@_œ"JÐ3?î…ëÃ¹ÿ?°Ý§Û¦¯¿êóæasbx¿éÙ—â¿ë
´Û¿¿ïýf],+UNASNone?Õ_ôøµj%?ÁÍ'ˆúŠá?Ô¿XH5'ž?ÇN̜hï?Õಿ=?ÄO­´'8?Í4ùi*=Ç?ÇHP¸²Ô?˽[un?ĸyõÁË?áÃjÈn?ÌH"K;?ѾÚÜÂ?­nҒ¯?ÆUÇîâãx?©&€¡›ÿ?áâ$ÙØÂ?²mgú›?É6KJZD?¢¨¡F®Cí?Ò<ó:w?°€Xªå
?à"o³¡L3?®¯l?ê°K4FGL J1454.3-3946?ìX½ß
@1<¯bk/À:ϳô¬æÀ<̙¡&@ýˆf# @ÿMzÝð?Ûô°@¥¾?ß?p\‰?ø)&i÷@´^»!S¸?ä»!©ô¿éî4Ïëe¿ãç ÏÃÍ¿ïÿÿ>¹ú?ïÿ‰ñÇ®?ã–!‰"UNASNone?î.:óÀ¶/?¯,Ž‰@/m?¡¶B:?£¨Ã\¥S›?˜!4‰Úµ?¥yR'²Qñ?ìR@²"!?Áj.¬ b? ‰æÉM?³'ûä³]?µ)
y@u?·ñ7Âe?ç­(fýPH?©ªX1ꋡ?µô‹|,o?cv=úÀï?ÆÊdL¨®?£"¾Æ
?î†ÎÝT^S?£
Û*¸(à?LÄxˆ¿b?^¤¿ž ?§ H™ÿÕ?¢Ð"g'lË4FGL J1456.3-5419?ﮜcVE@ي¨exÀ:Symª'†À;Ôj:0}v@Ið<h'@ž˜ÜÛ7Ê?ËOž"ë<?Ú6=©¯@}¦Z?þ)Þb÷F?êQMÀR@¿çœ'0>Œ-¿á>ƒö¿æ¡o† ˜'¿í«a·€	¿ïý\á0UNASNone?Æ/\zªÔ?µÐÈ_`?Þ§sMÚ ?Å,ÒáŒ?ÖÖªO§Oö?Âk¸3p͟?¼ÕÁøö]F?¶m²vIÆ?˔Q\:#?ÃOؽ/Õ?å€3iÜåÏ?Ãzì=KíÑ?ÔXì@…¨?­ÜÏXD ?Γ¦
·3ö?«Pà6
i?Ü]@¹à\?°À÷Ú1«?¼âÐ6|fP?™‰fj²x§?Øj^]Õ_â?·-»LD?à.vÊEÃF?·uB/ÏG4FGL J1456.4-7129?dú» :)ÀÀ&`®–À:ðª¦1W'À<m¡â=wZ@m®˜YR­?ÿ¶JêßÝ?Òk–|ÚÑ?ØEAþ}@pë?~›@uVSsÅu¿ïýРkð¿?ïÿ¶~¬®I¿âå{ð;g¿Ùó:à%Å¿êmbnŠ!W¿ïþÇ1¾UNASNone?ëk'ýߨñ?µÓ²̝2?"Eï!º[(?ŒUH·|­2?¿ÕDH"!²?´`ø6:·1?ꂎ®ö?Â¥w5gÙ?",ù94—ß?š#$Ùið?Ãp& y%/?ÁçH¾ð¥?è­À;?€³?«Rc'fT"?­1™^ƒ?"b‡ý¾¦×?Åü˜Ñêz?¦^]¼¦¸?èáçd®M(?£N"žè?­º­Æb?•i÷&N_?Å0~›YÇ?¡•*d@4FGL J1456.7-6050c¿îrH1ûƒL¿ùqÕëYÎÀ;e߅65FÀ<1vßZn@&£¨žð?ó­Â*²[1?Ê+?Éą¿¾Þ㥬Lz?öy^«‡ç@Êò4:o=¿ïÖHaÇó?ïí,•<=¿ì÷³•Ä"¿êzàñÇÙ?·4£ ®Œ¿Û­ë=ÑUNASNone3FGL J1456.7-6046 ?Ù[é¤?Ì¢ªvÝ?Wvü‡X?c	žMZ?ãFï÷.'?Ì£Eæ#`?³º–šÔM?¾'Q
CîM?€YO©/·?•V˜?íGGî¹ê?¾ÉGM
G?æ-ŠÁz"™?«ué;H?')x™òˆÓ?}ï—CYÖ?҂Rók°D?ªÔž<?ÀK•¢ùç¡?º«Àècp?‡Á¥‹Lò'?žip>Ž¡ã?ëŽRM?½±3õ4FGL J1458.8-2120?è°+†QÏ@@H‰ÁµA–À:eJýTTÀ<Ê8Ö?@ªqùílU?üäœ,ý?Ä·.jv–_?Ûë<äâÃ.@à8ýw"@p^ùÞ?ú¢É¿eQÃÂ)"¿É|ƺš¿ãÕô~A¤e¿ë6zæP+'¿ëü?¶Ï4†UNASNone3FGL J1458.7-2120?¿"˜ã¦ø?²Rõ»t'"?èÈÒú"¤?½0l©9š?º—hOG»æ?±"&ٞ×?Ö%:T.OË?Èd¶]6E?à'ü)…Žð?Ê:=Ëì5?Ámš±$«?²³GQ×R³?…ZÁ®t>?ª½†¡®?æÃGU‰é?²BwQ·ß?ÂmˆÌûd?¢½YVãõ?Þ~Dpü?®é!,šáò?Õ4]ûqF?°ÊEŽü\?Ț»'îõ\?¢õ7V‰L4FGL J1500.1-5846?´ Á÷T?¶j#¤
ÖÀ8®n‰J—À:'¤ÑÜF@¶ßªõâp@7րªµK?ËØF=&&/?ÈL«êªr?þ¦îœ*m'@%ýžü¯é¿ë¶D•[Fx?ì_>Sù¿è2í"ñÚ¿é¹Õ䣃'¿ê1y¿ß~€¿á´¬¯öÓ1UNASNone	?¶Á4ÚÇB?¯Š˜ƒÑ·?ĨœÂå·è?ÂÐØú!\?çý²4ù?Åûî@qö??¥''2­V?¦@ewÅÞ©?À¯¦Cp?Â4Êz¡?ê¡sSûù%?óÈ#¯?¹ƒ÷ux2?œt^Ìk?Ĕ=që?®Kráߓ±?窍`4Ö9?°?~}–íÙ?¥OA1F?ŠQÑRêC÷?±³WfJD#?žž|Ø??ìy#£? ªñÞÛ¤4FGL J1500.2+2640¿ÍºŒ';@N®"î9.À:ìðó®À=á{°z‡@ï¿ÿ^ðP@^@ÈG,?̈ѠF1?ïÿöàœj@Ú­æW¸N?þ äßh/ê?ïàÇ ½û#?ÖLòãÕ¨¿äáƒÞFqÔ¿îö'"׿ïö4osUb?ÃVú£ӀUNASNone?Ðw²|†.Ý?ÉeƒJÖOù?æ¼Î&{?ʙ)χà´? 9f×`?£Ðë5s?œfl,1üË?­
®ì¤"J?íéǨf?¶€þÍÑG?£0Xï_9?¥ábJA;?ÐtÕå?ƒ?­`|ÒµªÏ?àlš:ß7?±u]j=ç?Íd̕|ô?¬ê÷Çjª5?#ˆ,Å|»?rꐰuEE?ïaJnm,®?‡—TҜú?ˆ NR/?%]´¹B4FGL J1501.0-6310e¿î¾6ÃÀ Oœ'rÀ8AðáyÀ:c7ݼß@:<§P;'@¾¡žJÙB?¹ÑÓFäjù?Ò(ÝÚ;JY@Âl~®[È@ؐ$zß?ïÿA>8ÊÍ¿àzjÊy5v¿Þľ`xe¿ç§(bõ˜ž¿äQ¬šþ¿ïþi'O¦UNASNone3FGL J1457.6-6249 ?±ª‰Ç;"q?©Ãì0A'?¯!u¤sÙ
?­^byK?ëؗlÑP?´äòÃñ×p?µyW^Ý?³TÌPÈ?ÍGÐ`Õê¶?ÆmPKç)?åþéüè¹w?Ƥ@͂¸?»´F©I^? è·"À?ÓtWú'ˆ?±1Aô-Y?âÏK-Ž5?±¶ñäç—?¦WǙDϾ?—ç0•™ýÝ?°ïã;Rõð?£áW!÷9?ì|‡TF?®VîŽPD4FGL J1501.6-5236¿²•3$yïÌ@g¥ßøù|À:fž—/\À;Š]«¬Á•@®šǦ@ßæՌŽï?Õ/`àëgÃ?ãwÛÈgã@{6½+o?ú"1Ó·¢™?ÆÛ˜ÜZ^?èSðlõÍ¿åõJÖ½ç¿îˆÍ¿ì³ß@ñ^¿ïýZØ®UNASNone	?Ê¡"ÀQcÍ?Ààßc=Aµ?ÄãZ'Š›?½6üj³—?äÈF	å?Æ4\n\Ú?¹á+¿¿¯?·(^,C5Ÿ?Õ0ïoݺV?Ê»Òr½?âEŒ"™*ß?Ç~¶9‹­?ÐY½¯ð¬?©¤8QùýR?Çz²÷ V†?¦ïǃ‡q
?áôt¿ßò?¯ÿåì2ºÜ?¯ó
ñ=/¼?È3#$³?ÜA
–¡3?· UÌ,?ßÀ"7JÕ?µËÐDp?4FGL J1502.2-5933¿ªâ4&úË¿è×z:XÁbÀ:6›X¶z{À<nšèN3@ìÖæ(ß@yn‡PÂ?Ó|_…?ïêÇß}( @·zâm©@÷½Ñ²9Ï¿ïò¶kawê?ïû|ã€m¿Ü‰¦qï0¥¿á?ÅGMƒ¿íûª€qªg¿èÃà•®UNASNone?–0Áñd£?Ž'¶Ó¿?܏b^–è¢?ÈõÊù×NK?áMJ¥Š?ÈÌnì{–?'ŔeÝL?™ôÛcY?á…V<ìVÉ?Ï]Tó¨¦ê?ÛÐ&®ô˜?ÎäB"%>Ç?Å{ ‰
y?¤Ü ¹…žg?ßOÅÊÆÈ?µ%UAÕ?Õòj)t²¶?°¿"´ç %?œÓu'þÅ??ãíV5?êñÌ[Û?³^Q?§T?À·ô%D¼¹?±níY‡«4FGL J1502.6+0207?ïø¢áõ[•@Hï? §?uÀ;P¤J̓¬À<œ—w€j@ V"‰Š,ê?þ'ê–o ?ÐùùJ÷?ÃígaŽx?óy¡â=wZ?üjÔ²t[ò¿ïù™~Á¦ÿ?ïÕɕà§u?ï(¥:·‹ó¿åêa2Iÿ¿ÝŽè%Bڛ¿äƒÎSŒðUNASNone?ïÈAL•8?Œû³Að?BÔöýy?@IÛ/ؑ'?y"×Õ%Œ?Žáêïõ?ïíЫ;˜?ŸO-ó?gWa|F?xGÈ Ypâ?œWY»,w?œ,ˆŸ?íáß!HØ?'¡°=þ•L?~"'×>?s³l1 ¼¨?­'…Fü°?'˜'O??íÖ »0m?žÓCml?…u[]¢?3?‡ï}¢Ø(³?­@uŽiZ?› )m.b4FGL J1504.6+4343¿Ô™~aûã@MAtNƒÀ;±ôr{HÀ<æ¦qq@!:¾lâ¬?ûBr5§º?Þ%€W©4A?Á°ûàá'?ß¼[»g @^"'GA³?íîÃA³©¿ëZ=c7ݽ¿é•¢:Å?¹yÿöDëB¿é™RÀ—¿Ò½å=ÜÚaUNASNone?î—."ÇÜ\?¥Y¸V?hӜò†øc?t_%üV?¤ÿäYÊÃ?¤³';•5²?îÚ0R¥? äÿËF?c†lwœ¼´?qQ±ÂÖ?¡$™3\Yî?ŸüÅ¿="?íS/(‡P?™Zº\_Á?{9¬ý'ª?qì!誱s?³¬³$kíT?˜?.úęÎ?íµ_ƒª?œNŽÉƒc
?oÁnWöü?pÈBÕ_Ð]?±Y¹Ä1þ?œŸ Ãš4FGL J1505.1-5145¿êQDóœfË@WbØ<l˜À:P•,L%À;'(mÝS-@A—ȉG@R.»Õ-Ä?×ìe$?ãrl™†Nc@Æ.Z†^S?ý«è¨ˆË¿ä"œ!´/È¿ã)¨¥¦V¿â³CÕAæ¿ê…AÁÇ¿éèv¬.ǔ¿ïÎ0»"¦UNASNone?5ÄH>ñ‡?{œT–ç÷?–¯BQc?"ãW	àW?ï
3tÌy!?—J fŠà?ÊâÅ~iÇ?ÂÖÄĨÎó?Ä폚?ÁëJ¼É,ë?äA"`̓?Å ÌЙ-?Ð'ÀÿT?¨'‡½g?Æè±ïù™?§M÷ê~­?â=Š£¼ð?®¦œŒ•Š?ÁÜ"}¡p|?¦ˆÀçEI¾?ªaõÈydÙ?™ FR,	?éâØ
'?­M>%ÌЅ4FGL J1505.3-5852?â·:I°€Ä¿Ø#dn•À8\ëÉVjÀ:ïLS•©@ÊþOPË@l»Ý'@/?ÐLÌamb?Ú@Z£'®@ Ÿ°4?ùB)Æ"¿Ù¼sƒ…[¿éyq%Ú¿æµ^ñýÞ¾¿æ~˜÷³*d¿íú'
‹þ¿ä8*lUNASNone?vÐbóÚ¢?s%[`k}L?‰êŒú·-7?JûûáWÎ?ïjµ.–?"
6táa?¢6ŸÒÂü7?¡3†U&aÈ?ÀO•ßd<?¼Á'"¤§?êÈ°Šú¯í?½%*ò–™?¸G_Zegf?–­9¬"²:?Ä\:Eùð?¤âU2nÛ?çà'!Ԙ?§Riќã÷?ßÇY`|?s½`w8ú—?¨=‰Ü¡"?›ÿHŠô1?î4®ùüµ‰?ž§ô·elB4FGL J1506.5-5708?ï÷døö?𻦺Œ¥À9*#²Œ¯¦À:ÈÃB	Ì@ƒÇaÓڈ@@ÝûÉ9š?ÑP¸_˜1?ÔÄÃÿž±@FGwÖ@°s#Ž$›?íçòpËD¿ßÁ‹›T.Ö¿äD8¿HB¿âë7@¿ì*í+&¿ïÿ·`)
UNASNone?¸¿Ä¥r?«HXóՄ? Ö릈¦?²Çßµîc?ëñûMH?°®¶ƒ&Þö?¹Ë|ùvÉ?µrtú¨°D?«
ȱ6£¦?°>6âq™?ë¿¥Mfí?»Ö~Jƒ]‰?Ä+SW2@b?¡¡â"+[‹?Ç9)®÷.L?¥©ÙiB?å&à¾u¤T?©šãG5zV?¼z¼£Ù7?¢=Ž¡ë"V?¨HOošÔq?–¦`°•?êì8'qג?¨²ãCöN4FGL J1507.1-1901¿î)ôtþÑú@@©º^5?}À:Àh®?CÀ<)Táä·@ê+ÌâqO@œÃB	Ì?ÊK‰@[￲fCUë?è8)Âq)8@›oðRãÓ?í-$%y6M¿ê"`Ø\ù¿ì>â=ø¿Ä`‡êš"¿ïé¥J§Ãÿ¿Àø\È_UNASNone?ï"öQf?(¢±dû¦?€©ån'?"¤E׊të?t¡¹ú'´?qïøÌmã?îæFp]ça? ¸_,ôf?rB_âÂ?†âúž°09?ž²ámk?›š÷!e5?ìŠÛºIH?"Lm¤à?'Äðg${?"Iȶ…0¶?¶÷æ-" ?˜øæíŒ?î±(ÄhRå?"ÒçΠã?@"B?zì¢)×p? N³¶Q&?'Sb4Á\4FGL J1507.9-6228e¿è¡Ktü	À
@$ À8èO,ý"À;`CނØ@"`¼x{?û÷Oݍå0?°h­é\Ð?Uö´9És~?îz£q+3?îã!øÎ2¿ÂM%²—¿àWÕ©ë u¿Ú~½ÀjhÔ¿ÖCÐú®ÝN¿Ó"j@ºˆUNASNone3FGL J1506.6-6219?á°:ù6¼?Ê0QiË%?hÆóv©?c«*ª'?Üo€î¦~?Ê'Š¬1z8?ÆúDj¾?Ä[mÚA/˜?¡Ê¹e:‡?±¹º¾é&–?éaÌ«<ß?ÄöxCe´À?×QàS8F?±õþ¹ºs?£
Œ‰gUú?;2Áµ\û?ã&7-¿î~?±}Mƒ¦¯?ÀY¹¶L'?¦4ŽÝ3?¼ç
Ÿ"â?©va¯I?èL­/Þ|Z?±99!G(å4FGL J1508.4-4817?ŸI÷cÜðÈ@!)éBNYÀ:·o¿«|À<°}á­/@ˆmm–±@!#=ò©Ö?ØU-XþŸ?î┵.J–@ÁÀÊ`@ùï‰:Pß?îïŠ1FÉé¿á{À nŸñ¿ç³"âz´¿í³Y(B¿Ð†0[<'¬¿ïÿæŸÜ©ºUNASNone?ۊ£G,€Õ?Æqü'«Jê?ÅIÌ-ÅL?¿UsŒÚ	À?Ùç·Ò¼œ"?ŬÄk‰š?ÙX•z.†u?΅–Œ|'?Åø´a'@?Äfj*c4?Û«UYE?ː+ÉÙ?ågîG6èô?«Tº#‹Ý$?ºÈýå!»É? rHݳ–?ÌûÇð"~P?¤ÑàÒ)Q1?Ý°JƟ?¸Òïp|fÀ?Æp£CÜ9?¹¼t¬/¯i?×ã+þKF?¸Ùí'd4FGL J1510.1-5750?ïÅvgO?É7ÑÌÀ8àpØ°/ÞÀ:DÄ)B@ $ÀS @ZQ	Þ?Â*2	h?Ѐ{zõ"—@	—ZYè©¢@0oz¿ïÁ­)«Ë?ï'ÄþÍ%¿ã ®@š¤Ü¿åxÜö¼6¿êk7@7¿å®7¶O²ÆUNASNone3FGL J1510.2-5754?·v=ÇZ½Ç?®W9çô '?ٔ5ªëîâ?Ì°'?àGqž°Ö?ÌyêhÛ§?f´o€é?¡¼'Óá R?Êd$[ƒòz?ǜ}½¹Ÿ?è{ÁE£²?Ǟ÷æ[¥h?¶zœþÛã?–nÙ"u?É_ì3®V?«£1OŒà?æرZïØî?­k¸«]A'?˜fTSwÅ?Í_ãCUÛ?Âx`5e"?«è‰B¥ Ø?ꞵ:î)?¬CG²Zf&4FGL J1510.9+0551?î3é%ìâ@IM½ƒƒ­ŸÀ;IÝcpÀ<©7Ó«ä@ ¢§>H?þ7?öå?ÑWó;Ì^é?Ï
ŸÎ@ҘÀ¤ @¶ÙTD¥Ì¿ïùçýÕ®H?ïþY6Òúä¿Ø^m^'Rª¿âQ"ŒÂ¿×ÅÀÔqý¿ïüe"´UNASNone?ïÑíÃjh£?m!ˆ#M0þ?Yƒ"]å5m?SHÄ#pÁ°?p¨U³Ra#?gø>kSÁŒ?ï!AsaL?•ïƒ×1&Š?b/Ñú 8¬?k! Âùï?™'×T'uÙ?"dCô¹4?ív`xÇõ?˜å¢¤B×??•ªÌ¡×m?ƒ')3	\Æ?°''ŒÁJ{?"©±'JU©?í–B{•6#?•19?ô[Õ?‰Sgö3(?}oŽídO?°#B—ˆ…?"anæžN4FGL J1511.2-5803?ï¼B‹Zy¿¯ù ?{À8u–†¿¢BÀ9Ó²ÊÃQ@ ´<[Ðá/@C{~% ?Ö_þ"/T×?ÃWÿJ?þm…É=?ÿÂ+[xv´?éu^C,P¿é‹^e¿äˆHn-Û¿êÒåëÃº¿åm$€½ÕŽ¿ê¬ÄÉ$¢UNASNone2FGL J1510.9-5808c?²jýit"e?µ‡¹-.ë§?°<7º›;?¸e±Ã×ڋ?ë øËÚ?˜mm‰?™ÿ"#?¢ÚS.t?­ý:ªaçm?µLÏS#U?íTY5ip?¶çõ5…é?¶ÅáH®'?›"?¤£ôê?½|äior?¦3[¬?éÊ¶´Ü??©>SâH`?vù–®v"?cÏEgËj?–þZëâ°å?'ìë&Lð?ïÕ5s?'V"æ«Å4FGL J1513.0-3118¿åæÊ<
@6ƒõ@‰]À:Lm)ÏÀ<	Ä|œ2Ñ@ĐlIT]@Ý{~%ŸÍ?Ë®ýmS•?ÐÇ`&[^@Š#ÚМ@z6‡¦}?ë«6D_«a¿Ø	Žôúé@¿ä4߅·¿á'¼<[Ðá¿ïÿþ½à ¿?ï.°'kUNASNone?劥]i#á?À³&#3?»x!¾M—?±º%p‹À?ÌZüI­?»¿S#±?êT [U5?Àl$Æç?²\ÿiÊ;;?·?g»À?ºýý¹»?±Ý&Mw[æ?äÂgØÔ«›?°À~Ÿu^?¿‹%>ìÀ?¢T]''÷?Í0Íý6ñ'?§®¢AZ—?æÂÛ~ô?¬ÒéîWà?¬,Å´[Ó?"µO¦Í€?ÍéŒð—Ú>?ªR«)<»4FGL J1513.7-1519?æÀè¾x~Ê@A¢´A»Œ3À:õª®d,À<§)¥÷ß@_JÄIpŒ?ÿ×E|Y?Évz° F\?ÙÞš@
•ZÀ?ö@›R}PbÄ¿ïþÃT~–?ïÿþªJl¿ÖÔ]Ofo¡¿Þ´Þ. |¿êÂf͓œ¿ïñ.á"ÚîUNASNone?é&66¡m?¹1F¹qT?Å9†bº/F?¶±õ:MT!?¨¶ƒrÆ?¢"ÅXû[½?è©fڞ¨'?ÊÉE?¿Ú˜ü5/m?¾Ñð€@Äj?ºÚ0.Տ[?®ßÉIýˆƒ?ånO¹—¼î?²©ê…ÆšÂ?Æ»"«I´?®t§K&z?˹…õš?£æŽÛ֋?ä"{¢ž?­¢ÊÑùC|?ÍuâPðÓ?¬q8Šú¤¨?Ày·Ã¢q?¡Å&ÛúÓ4FGL J1514.0-6240¿×©æѬ
ÀÂ6ŸÏ=ÀÀ9Š»¬éØvÀ;6Û¿®×@S«šMÀ@WGC¸?Çê›ê¬²?ÉpNœ›+À?úzÞÞGH"@w9ÝÇEú¿ÓwÕd ¿ÖåoÛÛ£¿çUyC¸¼u¿ì"RÈú°¿Ôåî|b¿è©xŸNUNASNone3FGL J1513.8-6250c?ÞË ¹p!É?ÅÔmöw†"?'éGñ™òb?€æŠ:›þ:?àNʃ‡R?ÅÏIõsX?àBC9–?ÈD ÿr'?v¸˜£y=?†j2•(áŒ?ß ™RžEø?Ç鐖?ä,Åw,}?²"ƒRó%?¥é	‰©-?"s[-Ú?ÔéSଁU?°Õo7P^¶?æ¢ôa}?¯MòÃ"µ÷?Ä?ºKéª?pCO
iÁä?ÓVÍ».
_?¯&ü½ó4FGL J1514.1-5805c?ìÑ6'6ž£¿Ò"á#
À8ìÆ)wÀ:I¶>ëÎ@ É•½@Ï8ÅCk?ÄWŠ@
\$?(žÒ
?Ñ(@;Œ'?째Ex§¿ï¬^BUÿ?ïIë`á—4¿áu¿¿èŒ'Jÿ†¿àé¦A¯(¿æ֒³ÌJÇUNASNone>?Ä(y«ï.m?løÙtn? ËkfB?¢ºgNDò?éô4ä­~?ë:÷N?°ï¢@׆?µ†Æµ}õ"?¢zÆÎè×?®ŸiH]œQ?ìºoþ×V'?ºOUl?»ùAÿd?žC†~Ž±?½£^a¼u¸?¦B¢Ö(ñ²?èÌkóÛíf?ªÃ®žþõÑ?¦vªÂvP?•3ê«|€?£'ßžUx?•|®0ŠUu?í_wYøJ$?¡JX;"OV4FGL J1514.8+4448?Øòù}@L5BÙÏÀ9¾E	Œ³À<1¹[ÖÀl@
61u@­Ò^Ý?µ•¬O(Ý?ÅQî׶@Pó_ތé@ó̕ðB?ê_'Bd(Ÿ¿à¥è'
è¿âý ҈y¿æŽzí(8¿í-½R†`¿ÖNï|O0ëUNASNone3FGL J1514.8+4446?ìÐ]ÖÖNú?´÷¨²ìŠ?§"áu?¦Íæy¶ê?«f'.î?« ÿw4ð?ï.ì2Ó$6?•øÌû‹Åç?fÿ¦3áø?u0y?)?—B"Ñôüô?")4¬•D<?ìÃà#¤[Y?¢n'…V?©S_™=ò?›Wh(¸/?ªnž,¹ƒ?"VtqÎ?îî,"ƒh+?'N®˜_è—?‰f@·¢HL?s–{\€¥
?•‡OÁÖh?zŠNf¶Q'4FGL J1515.5-4242¿é¹''Z@)Zb˧2ßÀ:F;ÉÚªÀ;óò#žjº@€àîË¥@lè–Vîú?ĉûVxÍ?±Â2"ý¨?êVjÀh:|@üžîJI?Ҍùx&'K¿ål….¨‰÷¿ê@ý‹±yŠ¿âàÓ«¿è|ûhÁŠy¿Ö²#~4c_UNASNone?ç~¿uJ'.?½.+N7ê?¡n÷é¼?•(bš9ëe?Í©lÜôA?¼'€"ÅßÄ?ëæqfs¶?½yFðÙ6?Œ^«Åæ"˜?š0ÿÕV?½@¡Œþ?»l—±´ˆÞ?èîî B?¯>rh9?¥.«2±9?'åoc+ï?ʗùÝxÒ§?«ò[Ô¼&º?êy팖<?Ÿ•)lµå?–±##À¥"?z–.¨îXô?ÃB%i/žZ?¥æÃø1O4FGL J1515.6-5817c?ëôQR5µ¿á̓ ٔ[À8éŠÆ—ÿfÀ:'Œri©è@àØÏ›y?ÿ›¨g'¶?ÎçŽD%ô±?ßϏ_Yø?õ,+l•T?ÿ –H+gã?íu'}ô!¥¿äXYÐUî¿ç›Wã¿ãâæIu"Ø¿î]%uŽÛ¿ïîÞoŒÖUNASNone ?†å<œÎè-?"Æ>9þ:?c"`wXu÷?eÅÞcZm?ï×­ké?†¯Úz²?¼&|¸!#®?¶ÝÌ°Yc?˜ì™E-Ñ?¡ÒžÓLî?ë³ËžÒm?·^4N.¦+?ÂE…š>h?¡£Úam5?¤‹Ä¿X?¡íC¬@*?æÅ{Ù?6$?§•{&*ì¹?Ÿ9–ú£ŠH?™¥­ îÈ-?'y~šüº?'°aøA\?îrk6È?¤:En¥4FGL J1516.1-6429¿íYoÕGgÀyԀö4¥À:Asqç£éÀ;¹ë\ÚÌj@c¢fǵ@ë'Ü5ö\?Ôvóý=Wú?Ù%ñaËØ@R$ZR[í@…ÉêoJ?ï×"ÆÔeH¿àÛ
bY'l¿è÷ïÅöö¿æû	 :2+¿ïþ,@OÑO¿îôÔ#&vUNASNone?ãst?Æ-šN?Æ·á*>Ô?‡ê5ºÐï?Ø+''?Å÷ZwFiÚ?Ô˜"õô?Ä$¬ê»ô.?•aH@NÝ?œLýœÙWT?åLfï䂎?Ä6M#WÐ?ä)§9µÏ#?°³Ԉ.?´þ"̍‡‰?—ë"£C"?ÒmYpÿØ?¬ï&F6?àï"X%;R?¬¨%Ÿµ Í?¦ƒÉHyƒƒ?'Ž]ø˜"?ÛP^&¦Xê?­–Í»F4FGL J1516.4-2640?퀠ÈѯN@9âÀÆ.MÀ;':ûÀ='ÛSxM@¦¢Ç•«M?ÿŽêéîEÃ?Ù¦û¢"T>?ïx?ânÂ@
UûÐÆW@4:¤ì‰¿íŸXàÁÌ>¿ë5ݜþ¨è?ÖȾË,d¿×wß4®]v¿ïÿëþ@bF?Ú>‰¨ŠÎ%UNASNone?èÁúÞö×?Â\"|«»?¾VY¼ÙÏ?·©_T¦?»ÐØ·Ko?¸Ón«÷?å"†>ÿ?ÌoUfC?ÊgH7žY?ÉÐLõ"V?¿›=˜Ê²?²ÍUH[?æãqZ¦.?²d4bEþŸ?¾Êé?™?¨à%­&úö?ÅÆG{?©®¸²¬B?èï
oìš×?¶(ÒEÃv?ÁºG˜% ?²•o5Â3D?µPPé1?¥XÉ3•%<4FGL J1517.7-4446¿ÀϘ¹þG@%w+#š8üÀ9Œ)s–БÀ;ÔÞ]	@³6	Qbs@ ò{²þÅ?»õÔ­ì·Ï?Á$HIDíp@hÚdeg@uó>#§¿Îú1^ò©«¿æp>Œ,ɍ¿ãï
¿[J)¿äÍLN+Í¿îM"¸aþ¿ï÷#M"MUNASNone3FGL J1517.6-4442?äc_Ýá"?À £Èër?µ28N,?­/ê#!?Ñì¹ÀÆ)P?¿ÚÅ0–"ä?æ̦#Yñ³?șÿ1˜?ºI‡RÇ?½LE
ˆ¶ë?Ǩ¦®ï3O?ÂçÉÔÏo?æ—íÓo–?­iT>…µh?¸¾•þ£? Ø6Iíæ?ÉD=Ç.BY?¦q3wôŽ?å¤dSäõØ?§‹‹ÌÂ?¼RH;ª¤?žÇe<L:›?ËEJ'–Ö˜?¢Éȱ{Õ4FGL J1517.9-5233¿è÷ÔeX@'Š^"3NÀ9….mє³À<
ÇÚÅ@…BüÔÒU?þpCÊZ+Æ?¾q)¸á—?ãssÊÒ÷‰@ —¨mqó@‡B¨œö?ïü'-ks?î"=ßßy"¿ÊͲûÀUE¿ãg¡yâÅ¿î—;»—ñ#¿íÇîÁ"4€UNASNone3FGL J1518.2-5232?qýÙÓSÔ¥?v-'aÛ0?ïXM<êT?—çó
~ñB?€_ãÀI?"¿™d-?8ƒ[mµ?§BÏÆï?éñT¬¾­+?ÉOÑ>X?Æ3ª™Ýœ?Çt•NÃì?–Îè V?¬HI>?ì°Y'é?¡£¿:'×?¹¦ú9h°Ó?žáº®ýüq?©ôÕL?y•éDOp÷?ìÂO¼fª?¥9ŸU~?¶;ÞJN0?¢Ï:Sò£¬4FGL J1519.7+6727¿ëISno§á@EòxžwNìÀ;5Ñü·v#À<ùm"X9@ $©iuÍ?üGÐ^QÄï?ÌJ?(ßÈ'?ϵшžI­@l6|"ÏU@t§^ÿò?ï˱^²<ÿ¿îz´0ô"'?ÁXée´º²¿×¾Nî÷ð¿éJO^âäf¿ãׅøÒåUNASNone?íY¨§Æ ¯?®KNÿ(?Š^›0;qç?'éR¡É.Ü?±æç[njJ?¬c¬ˆM
?í«&ɦ?¦Èps œ?"™6?G?†>-
jf?°­"ïߨ?¤u'»	,?ìƧboìÍ?›$¯×%Cî?'üJ‹	?d?†%Î0©µ?µ²I¾IÁ?–¤*Îa¦?ëql"ÖRã? v¸^´½?¡ïJÚ,9?O ÉT[¡?»}CàRÆ?œ-24FGL J1520.9-3805?²xn@/÷ûH
ZÍÀ:}ke©¨À<#d"@‹ãJ<º@݊ú`"?¼+ö}ö%?°³'i#°?ñùYˆ1'I@¬ø¢¾†c?ïÿ™¾, ó¿à]d"Õ»¿é¿VŒÔ9¿âðP•CɃ¿à^Æz£4¿é9†3‹GÇUNASNone?ï¿=»è?£…0Ä¡?d-lô´(?] ¯Ì
¼?œâjªÌo?¢à<µ×O?ïD‡3Ç®L?"ö—·LÏ?ZM6Ló˜×?ohã7…‡?•ÊF":üý?'W£#,
?íwÖ	_ô?™‡Õ™Ý|?‡•pI»£?xY·‡<Vý?±N¡.ËÈô?–XÚÆìÐ?îMPË="?…~\aîè?‡DÂÝe½}?pË#dÑÉÒ?¥Y"ÎP'?'ÎÎúê
@4FGL J1521.5-8057c?ãåƒ2á
À3Ö/'4ø/À: ÃÄæNÀ<€ãÀ.@ÜaHÅ@¼@cÃb(?μz-È?ÃÏeÙM¹œ?öɊ=D
@™ÎwFÞ?ïó¤r:¯ÿ¿è</áoA¿èm`áAMþ¿ÖV¨ƒAh€¿ð?ï÷vG…UNASNone ?ï3MÎÎ?– "X:à?s²È˜7Ý?r*q¸¿.Ã?"©"—Á?"aod˜c?îjОåu?¦þy¿
Ž?}oTû-?Š–g—¬š?¥¥ÕkrC?¢³ó¬çˆ?ì8©RùtV? Ï.ïPZ?'ìvÄ­ão?'wÄè"Íö?¹—·äo?É:­U¦‡?ì3a…ô~Í?¢ó¤Â¤q?ŒãAs1Å?|9Yü›öc?ºá×h-£`?¡ãü""4FGL J1525.7+1503¿îI঍@JOKD¢À:€øõJÀ<NúìšÈn@$¿÷t@öڜ™(?ʀµ^å?´C_Bå?çváfÃ.@V'Ìx"¿à'âLÒ¿êp'_ÀYø¿æ܀w¿ïÿ»6¢S|¿çlÊcfæ?ì A¾ç0üUNASNone?ïî|iä'~?b–C;sŽr?B…J¡?JˆËÆÕã?Yć(Štq?_ýTðO'ù?îœÐÂì¯Å?«e˜œ––ú?pþ•Y?'S«JÍßò?¤1SÿBX‰?©Ó¿NµÙ?íý§2ê1?"úuEÙÐü?ydGѦI¼?s`DwSg?¬ùBœ"®?'{¯ðKë)?ïœe'¤¥?wºÇDóŸÄ?WˆOË/Í?P/ÛíP·?†®MðÔ?v)<3Ïgä4FGL J1526.3-4501¿îÁZ +üU@#XO	RÀ9äù8¶À;óé Àiè@;öófêp@ƦºêL:?¶z;°ZPY¿Œ•¢­Ù0w?ÕÁÔKFOp@'XŽó£?瘝N(ÿ¿åÁéå‡ó¿äâm©PÇ¿âø£JƒÄ¿â":‡»JÄ¿Îi{CÃ#VUNASNone3FGL J1526.3-4505?äJ Àh÷^?¿/¶KP³?E¼¨ìß?
C3ÓK?ց™æ±=?¿/ Y­í?áû$ŠÉL?ÉÞ^ïýí?‡",y?'I/~£%î?ÛM}"?ɛoKaòÔ?罆¬s]?ª"tK*Âz? ¦³XĄ?…Òz¡QŽß?Ï© 8xm?¨Ë#¡ò?èy†c"?£ŽCZ6¸?›"óMÛCZ?'\Šæ ?Ê©yT+?¢Ð–ä,JÞ4FGL J1526.6-3810?éÐԞ¨L:@.Ž­=%$À:ŝ%Ü3À<°ùïDÆÙ@ÊI±Nìø@l ºŠ«?Ê0pÍ¥»?å}¦‰l$ì@‰¡vݬï@-hŸ¦£î?ïÕ'^éšc¿â鏰â‹{?½Á]'çüS¿æ[Ûâ¿¿êíò·B!
¿ïæfÁ«¨UNASNone3FGL J1527.0-3804?ÁFßfË?¶¢$ÇöžË?狀ö5â"?ÃÖøO¡ñ?À‹ì?½o½G{»D?ÆvªõQÝ?ÃW2BN«?äVÇD%?Ë¢J•5Z?Ésùî}ސ?Â\Ë:h˜Õ?ɀ˜2‰àµ?¬µñoÏÀà?äÂ6ý×)‹?²uʤ	¤2?Ãv‹Öy?£}ðõ" ?δŽôÃ>?­SRb7àµ?â[
–?¶ë'?ÇßU¿øän?ªåuú4FGL J1526.6-2743?ãH(zóf?@7®8ûÊZÀ:³*¸:n'À<¥Ãiv¼@Mâÿi,>@mæh3?̎BM'iÒ?ìq='‡­@ó'ªi@éR ‹Ñ/¿ß´[ÜõŽã¿Üυ
ñZ¿ÆGçà¤p¿äšyޓHÈ¿ïÿÞý¦ßR¿ç#î¢	ª¤UNASNone?³¬*êÎ?©GõëG?ëuŠø€&á?´ÖùW¤b?°§¨úÝ?¨·CÇÂý?¥ÁË¿5&Q?­5gý¦öé?íMÒ{ʋ?µó'⏎?ª	W0ÿ?¤òrí¥æ?À5±äâ?£k²ˆ°¬à?çˆÉ®Ïå?®Ã¢Þׁ?ÁÃcÀ'Û‰?¢
…z%Îý?¯Ò<×w?˜×ò—?êå)†¥¦ˆ?¬[Âì÷?¹V'á´_þ?¦蔘4FGL J1527.3-3103?Úü4É$;@4ñá~4¹EÀ:åJrÀ<%1ðÃ@ú"\ñrŸ@Õ7ªÉ?Á·]ú²
Y¿"ÝLÌ·S>?Ô »¡×+@t³Pw¿ãÓÇÝúœ"¿ÐùW¥ƒh¿ìUŒŸ
FÖ¿á­IÿþR¿×Ōf«/ĿٙޣcòÄUNASNone?ìAíLÑG?´—>ø«‡å?ˆ,5ÛyµÅ?ÏÖS0Ãc?ºñ©Ú*??´õfþ‹?ڬ·?ˆ_ܵØZ?G¢(–Ã1?U×®+Ë
\?Ž&˘Eà?‡KÌ¥?ëõ&TJªD?¤Ýƒ½Út¹?c¹Æ›Çö?¶1›¹Ü?¼=Þì»ç?¢Ë'n®‡?î[
´P_c?Š fY›üÂ?c€±à_?U–h!Þ-?©$oÜé?Š'âè;­4FGL J1527.8+1013¿ïdógÉÆf@HÁ´xB0ýÀ:께Çâ'À=ÏZ@Ѧ¦G}@dGšÉD'?ËãŸ6¼£?ïþå-7@''¡.¹Q@ÏUï˪c?ïöW	ÒÙ¿âô8ñ
¿¾Ôw»ù?ò¿êõ°»õ4¿ïþÈÈ[N¿íº(ðºßUNASNone?Ôµ~KÔ¼?ǝ@Úa?ã@o´øs'?ÊP(ÍH,?³(_
…?²°pm"c?¬8'!Ž	?µ5¥ÒŸ›?ì!H{ȓ?À®™Ä¥"?°Ùs­e?±@o¹
_?Î*Š(>'¤?¯aùŸŸ²ß?ãEþ#G˨?²l¹1ŽÎÙ?Ľ}J¢?½?¤½²°h¨?¢8€A›:"?""=:½±ã?íÈ;êï'Ù?£
¨%
R;?¡CÁk¨L?˜äÅ]‰Ù{4FGL J1527.9-4943?íAÿ©ÃÞ<@š¬"¢ºÀ:N õCÀ;‰Ö,Çß'@"zvž˜@öuÂú»ó?Ϝâ#v&Î?Õ§IEbø@†NÜ%´@£E9›N?ïÿèã«6¿ë3!à¥q¿¿ç·€4mÆ¿å9ÞHT¿ïý6âjBê?Õ
‹ÄCç6UNASNone?ÓD{Jʱm?ŏ¦yº?Ž¼'Kƒ?‡?}jQ£?ååmÿ¨^?Å®jÛUˤ?ײ'{¢—Æ?ÈæàÂAÕ?±Îëð{TÛ?²_mµ'|?áìáDI?È¥këåp?ÔзƒY¦?­,Ä«4ÊÖ?Á0'ðÉ?¡omp³1?á0d2–û?®£Ì ´Œ?ÛóãÖ#ï|?³b/Ç%?±`s|#–?—ŠlÖ>̔?ß³ÿJÓHÞ?´0ê¹pÅ4FGL J1528.4+2004?áD¸/ ›Z@J¿
=p£×À;møDøÀ<"ìˆ3@@ $¼ev|^@¢€…Ì];?Å«®o´¿¯ûÄÃ$=³?çžQYŽç@#+¿÷Q[?í¨)µ/ë¿î±
õ´M?œÄ1%oƒÏ¿ß¸ªŠ¿ãbr†/YŠ¿Ø#lÁŸG.UNASNone?îS/-äš?£Qjߑ?s'»¿÷5S?q2aI¨ow?¨[å•"Ͼ?¢¨â¡2k~?îÅ.¦%†ð? †[ZËó@?e·óøëE?re‡´Æï8?¢QœžhZ?žï֋—b?í"|z€Ô?˜3w•…h?|Û∌©Ó?qYZVaËâ?²^vþÁ?–m7þ§×†?í6fšÙ1?›e³z'So?|'7Êç{?rùÈ/+"?´ƒªõ»Oü?š*`Œ _4FGL J1529.4-6027?æ>l'­õ¥À
ª'†VƶÀ:wP™u‡À;+;íìØ@cN€ÌC@yDàá6?Ì0_ïÉ|?â)ñk@«ýq°F"@ü¦
›I?ë–åõ'¾´?ä	Ñ¥y¡­¿åœ,ñВT¿éËÕ¡1¾i¿ëîjáö)½¿ï#ˆÕü÷UNASNone?…Ñ,"ÒÜN?|>Ó6(õ­?µÌ=ÖöíË?³2®ñ-?ìï3"
ÖÕ?³Ã!2®?Áàæ%´3?·x+<7?Ád'Ÿ®«N?¾Rybg†?çB§Šè ?º ²íƒK?ÅþzæÆó–?¢ú_õ¥Ã§?É¡w~cá?©²ûiÎ?ä¨nª#?¯(Š_ˆ‰‹?Ì<.¨aª?¥~"§i'l?Ó`«\²øs?³Õ7|œÝ?ޓ¶‹øÖ¸?´ĔÜÀ4FGL J1530.0-1522¿Øù8ƒ="@@V¤"‰—ÄÀ:°úìšÈnÀ<Ò¦*¡"@ÎÝÉl@žnëp&?˳+;-C?ãõÄ<ÛS@¶'ö @0W`¹ÿ?ïžæu¿±'	/(·"¿Þò¢¿æX~FVüf¿ïÿÿ&¦³?ïYÌ?SŒUNASNone?ÍÑ0ÞÜ­
?Àš²BÄæ?âÚ[4¨?ȉçÎH"¢?ÆÅbP´²Õ?¿ &kŒTp?Ññ·…%?É9ûÚ)°?âм8%š«?ÍÆåX ?ÀÚÿ°_w	?´Ö8õÏ?ÆÝò ˜¬?ªqèSÐÅý?ä{îÊËâ?³}Xø^f°?Ç3<â¯Þí?¨$ãŸâv?Ó\G¹L£?±I~"aڑ?Üۊö[?·of§S:þ?ϐZ¡)Mš?®'fs 4FGL J1530.5+5850?ànŸŠ±@H
r!…‹ÆÀ;0mWoÈÀ<­
‡¶B@´×xÍFD@b??°ï÷?ÄzIÚÕ¿¨ï¥È /?à>¥ÂœÈ"@çòiÇ¿â"±?¨Œ|¿çº=³¿µ¿ék¥^¿ÿ¿Û"à?¿ïüc]j	?ïŒËà"©UNASNone?ïÆ1a¡ˆå?vBÄØK¶r?nW`EoÑ?løÍO‹Å?kw>d«E?i@´'
Œ?îîWᰅ‹?¢­B®énÆ?c…è*;?uy¸ßž…ç?ŸÄFnj©T?¡Зø‹?íøŸ§+?'€7ï3?…í]AÀ°?t¸Á
4Ù?«=tŽµ?é%%·{Ù?ïáûCŸ´?{K<iA?pEü_Ïëò?d"ԁ¥ê´?‡ä'ÿ0ã?v#	·4FGL J1531.6+0406¿íËñ]OçI@F³åBåWÞÀ;VÔ"+¤À<‹Øž'&ß@
8=3<@Èáž)?ÎFacGM?ÃŒ¨šhw?öFl{S]u@W‡§£?ߪ_d"(?ïñgìxc¿¿çeà"œ¿ÜâÅB>ê¿ãžzߚ.ë¿ïÿÀ?ЀUNASNone?ïT¾Š´3?ˆ¼Và4ž<?fUn'gh?`8mþžk?'‹¹¬®?‡qö)M2/?ïU;;Ï?'ÖއH­?V"ÌÓå[?bIA¯ïöµ?"ïZÛÐÃ?Ìêl¬q¹?î5êè ?ŽÃV5e6Ð?xµ$‰¼Ór?gEÁ–ô'*?©Š¹ý©ã™?‹ÑÂW>û?î h†j' ?Êõ½À)?ˆðÀ³du?wå­lÕÿ?§½ui)üî?‹S)³À/4FGL J1532.3-3857?ÞÞ4dô@+ù"pŠ¬—À:Ò«>݋aÀ</"Bð?™@عó¬4§@Iß9¶Úó?ʽ	¶74?°"ŽJ[?çÉ[ÉTrH?üùä]K?ïø¯^|ã¿är5<!ï>¿æBµâz‰¿â^06ÿpŽ¿å'Ë9NÖ'¿ï×G²JkUNASNone?çôÒ«"â±?Àä–vMt«?xòw &T?rn⁔ <?Ïe!–p|?ÀÊb˜D"?éˆtS(>è?Å°åBÉ{?‰¢M¥Eý?'0é$ZV?ÈD
þ?Å=}Ý«?ë¦:øK°?¤,D~¢ì?'©)A5:¥?€‰_ñ_˜>?¾dó×ðSÓ?¢K¹‹#ƒ?è	L'?¢û=þ½…?›Søæ­Z®?ƒp'š6µ?ÌpP²¸L>?¢WìÛ·j»4FGL J1532.9-0313?Çq¡|€È×@DR)AAé¯À;Z4ù»À<ʽé:ø@4ê˜d»@¢®Ñ9C?ÖTéf`‡)?ë6ˆ™"º@	 &5@H8}õÏ?ïå²af¢K¿å±ÏñD{Z?Ók—}µk¿ç¹¾!ä+c¿ïÿ¿h`;ª¿¸_ô‡PíUNASNone?å…u¾òà?Ã'0–S?ãïŽy[?»L©•2?ÆF<›u»%?»7hÞlùþ?ß[/~5ö?ÑYÚ-×l?×1LsJ¥ª?ÑùÁ®šÚy?ÂçÞnH½?¶9–'¥ã?å4þd ŽX?®¢`é">?Ã;¿©\#á?¦§¸øˆÇ?ÇðFÆ!¢½?¤Nv'H3?ÒÊéô÷ô?´ˆNG'@?ßêÑJc¢?½-¦ù_á?ʔ‰ƒËî?³_½c1"4FGL J1533.0-6239?ïÈ­øeÑÀ†¯f•À:w
)´.pÀ;¬;Oag#@ȯ+|/¦@È˛te-?ÛÜ:¾lâ¬?í:û@
þ
A¢a¿?þì¸"ÁE?ïâ, GÑ¿Ód~d‰íT¿ì&½F¿êÍì‡}7c¿ïÿØ]#Dž?ëÛu<Z#UNASNone?åöH×?Êvö­¡úN?¬¯	vRˆ?®•â°'?Ò6"A(?ÈÙl›Y³?Ç5c(1,?ÆmS¸µþÁ?ˀ×YÙï??ËQlæãŠô?ãRq_}9+?Í6ZCäµ?×Qáõš?®m¸¹n"?Çïù¤,š?§—¢S.¢?ܶ–å8O?¯äA3ÖÿÃ?³r2{.M?¡?U®	?áþ³eú?Ãoò¦uò?×&—k¤?Á'É°šÐ4FGL J1534.0-5232?í"í•Å$@QÔ=ÚV"À9—$tSÀ;NѼÖ_@¨a3÷~Q@f":Ì?½-ݳÏи?͛ƅ
ƒ@P +"?ø±\"±*¿î	\Ý°Ë?ïûPÙ6g›¿âÛÏ3¯Yõ¿ãðV+Ü¿èÏ}¶åû¿ê'úhçJ'UNASNone3FGL J1533.8-5231?Ɯ‡†ºÄ?¸P»ýŒN—?Òµx 1[ˆ?ÂÃm'¥0™?àþ=ΣŠ?Ã`²"Da?¸¾¯ ˆ¼¶?¶®ß˜C¸?Ôhü§úm?ÉÅHˆ>ž?ⳫÇñÚ²?ÊOș¢M?ÓO}`H.?®Œ¢ûÈ"%?·:Y›Í>?¤$=‹aN?᪪*èèš?®YÜc0?Ç ÷Éí¬?£í
PüDÛ?Òµ;OØûä?³ºW¨^ *?àÝ$e˜>â?µ1–§@4FGL J1534.3-3312?Ó꜍â"Â@2WÙÛ©¢À:ßØy©9JÀ<~Ú©.b@‡‰6õàl?ýL¹ñ'ö?Ñ»è#'?Ýp¥°@
E^³¾@oµ9Þ,?í`L•ÚȿڅKCuJ°¿Ö…ÜãÆ8‰¿Ú'}keª¿í²Ûe¿ïñn7@UNASNone?çŒ-²fU?ºìÿh¼B?¼Re(ÜÉ?±xóõК?æªÓH?´ý¥:®ç?êèÿÄ£?·ÂÚ<Ë7£?ªå/üð?¬[‰)<Í?»MQêUr?°I'§Av?ç8DŒÜÉ?°¸ØÀÍ4Ø?ÁÙ¤?¨Î)Êҍ¶?ÂÏ.¶=?¢×ÛxX³ó?ç—ÉÄ a?¤‰•âÒ³?°ÒœOo?—LxíÉØ?É:º
ŶÆ?¡Ê//¬24FGL J1534.4-6719¿íeE«)ôÀ"ÞøH{šÀ:ª'ݽµÙÀ<9v+ÖG @zJ''?@(:6?ÎRçÃô*?ÒqÁä;~[@m^!ôFŽ?ù´à‡iÁ:?ïæ†è¼í?ëP›ÄDæ¿Ù?""Æ¿äHcUeb¿ïük 	ŠÃ¿ïÿÄ;-ÓxUNASNone?ãtC¿h?Äû °ÅPó?µ#|¦¹?°WœÌ´¨?Ô»™XDé?ù¹2í7?Ќâm3ý?ÇÏÝpU;=?ÀˆOA|-¤?À¼ëN°™"?ã—Ü>jZš?˗"Çíy?ãûÝxhõ?¬pÈÖUnƒ?¿ê,o½Âð? …j8!Ùv?Ð
¹ó>¥?¦ßkÐÆ3Æ?ÕöÅïno?°n…_îï'?Õ>ML`!?·TÝOLøB?ÕA»í°p‡?±Ž¶Ìþ_§4FGL J1534.7-5842¿æ'ÚÏ*0fÀRzÊÒÀ:¡s¥ê	ôÀ<–:º1¦@ 9ʆÌbo?þð– ÀÕH?Ò)0æQÙ?ïþ©Þá!n@kpüÂ]Þ?úô?Z2üW?îôÁrüvß¿è
þraF¿Ôsíw¿Ð¹PC9e§¿í²UB&Á
¿Úk ÀÀUNASNone?Ãá^H;l´?¹fÝ®ph?×!àaøûa?ÆÙi¿¬i?ÞípyéNE?ÇJýi­? FnÁÓjú?©ÉºÆ9	Œ?×HsRX×?Ðâ ë*«W?ãW_j¶Èå?ÐN¸!´»?ÑK¨–D|Ø?²¹mee'?ß9¦œnú;?¶'eÄA?Îõaš™Ù?ªO½MYÀq?œXdèâæ?'Gž<Î?ê9ñuáxÝ?º#bÅ3­V?Í-‹]ÊÎ?·Rðñ¬A»4FGL J1535.9+3743¿ã\1÷tŽ@KNã'áïÀ9瑳ò
tÀ<"âɎSë@–íÐÓl¤@™Ãیƒ1?µ
A\Õ?ÉiÊßaÏÔ@Ï8ÅCk@ǯPY?ïjøœ^oø¿âûµþ!s¿âOX}o—h¿ê«³AáKà¿çv"|#g
¿äk_ý–™UNASNone?ïs	•e	?‡ªØ|?†ù¾p#?†Ôeè9X?zTQÁЛ?zR¹}QªS?ï/"™qŽf?˜–´!e¼?cøÊ6üv…?tÁÄ
nޅ?—ŽSŠî¤P?•zÚ7U-Ô?í/͸TŽ? dÂ'ªFË?¢Xï°¬Âì?"ÞT/`?ªª?Íô'?"Š!¸æS?îa©…O϶?'ÆÁP®Ð?Ž8íB}¬Å?~=ŠŸ7¸!?¢W,Zc™q?€­çžôz4FGL J1536.0-2729¿îƉ"Xï@6"9:´0õÀ:×ÌQ|ÊVÀ<I"G!þ@dš½."@¿]þ¸Ø#?ȑ²ZÙ.?©󼥸6?âȕз=@rƒ.H<Û¿á#bp7 €?ëì²ÍOÔ¿éj¡3–Û¿Õ6—;~Ü¿ëé[x̚x?'E¿&ñÜQUNASNone?ìp|ÍÃô'?²i`ƒ%a?ƒ°¦W?|"k3F9?º#'K"è?±ñ±ÖΓ?ïx9¿í­?Šô,«ØV‰?Q_/K6?]˜S KY?Å¬þ¢±ò?‰W	o}?싀¸Œž? ,yÏ~Ã?Oy°Þ!œ?€7â°nt?·!n¬?œw,UüÄ?î3£Q²ö?Œ¸2»Ë-|?Ã`Ý$³C?jÔ»þJo5?¨Í^É:ªD?Š¶ã=4FGL J1536.8-4327?â¼#±#è¬@#·ÃøôõÀ9­‹0JJ§À;¨#ÃS§G@¬º†¤ƒ@™åóí?ǵrþzCé?Ó4# Ál@€IÄo0:@/¡¨Ü­•?ï¸\Ó?­•¿ãšµùK°Ø¿ìpgÁ°9¿à™¬cû¿ïÿ݀y7$?ê|'œýÒ(UNASNone?ëÅ[Jó<?¹¢™L¥BK?¦ŠR¯ ?§ö…Ì'֌?¶È`j×P?µ>€›U¢0?å~¾7ƒ"?ÏËý™™"É?ÃSNO)€5?ÆlàŒ‡¯f?Ȋ¶·øq{?Å4ýÁŽP?åeç*þ´?¯,Y!)Ä?¶~´¤›ü?¶;Äþ·?Ï)	H5S-?©6)µDÞ?çŠ2¡á?°¡ÚýÞÐ?½5&j¼?¦ó½BÚ՘?Å+D2wÃ?§`Tђ>4FGL J1537.3-6110?Ù
^g¿VíÀåë`5ʽÀ:¼înÞ-À<5ÈÝT@9ג"­@N:Wê£?Ô#";9?æþ
·x§²@)@þÍÐÙ?ú¸6OL,?ïýi¸*~Y¿æ>
ÝS­§¿Øðh]a…¿èWJ*,¤¿îÓ6=ª¿ïȀâ¾|UNASNone?µˆT@ÌÏ?­ÿyáå…?·Äõ«™&?µgÎÇiºÞ?êVV‰¤b?»É°	ªk7?½1ºŒôò?»ó°^]®5?¿·‰aX‹'?ÁXð0'që?èbׂ6l¼?Ã
	"א?Õô£_íáÉ?®ˆÙ %ò?Ó~JýHÑ?²khÞÍâø?֍¢Êe?®?Ø=@>û?¼áVæ?˜ãS忲=?Ú¸ƒ2÷Œ/?µŸ^ÓüvÖ?Þ8	rî˜?´g.Öè\4FGL J1538.0-4638¿ìÉGß4$í@´À>IëÀ9¥£×àýÀ;V$fÖ@Mj¾È5@k#Â|ç²?ÄK9?ØÆÝ"/€@͌ƒ"_?÷΅Sç]È?ï"ßµ§í¿ärEb	àT¿æœ­äª9¿êðz¼^À€¿ïù¡¬'$¿ïïæ­H£UNASNone3FGL J1538.4-4656?ËÎÊ鹚?ÂÕ2°äBƒ?ÈD¸‹¨?À¬K‰žXö?ã>û"Í°?Æá=T"
©?¶U»‹#g?¼ÎöçîFý?ÞD™AÈÙ?Í2ÓPsY8?Ü6i÷ÛnL?ʍÕӍ¹?ΰîÓŒD?¨í`Ó6‰B?ÎêËU´?­â"kŠÖñ?à™u÷¯î?°iOJŸ1Á?'Ý҆±?ß?u0oF'W?߄VÖÅ?³e)#=
Ò?ßMÌу=?³ºU&á™4FGL J1538.2-6201?焻ž|,vÀåKþSýÀ:%™kvqÀ;&hI•u@dð9äRP@˜ þ?҆¨%M—c?ц^~e‹ ?úoŠfö¯?û:+õÒ*¿Õ<â^"o¼?ï£éIUпêoÞµ,¿çÒñ©ûçm¿é"µÏZEÇ¿ïó!ž¶9UNASNone?ÑaìûƒM‰?šÖA:~?¨ÉYËÈKó?¥5hö+?åÂsåÔ}?ÃÇïÔ·µ?ÒMX¼ìw?ÅM<o"ҍ?¨=RÉ7?¬á5©0‡?åXÌ"vT?Ç#Ĉ" ?ÔIà¶?u?­E&î•>?¼Ô¡GÆb_?™Ú@~Õ?â@{{ç¬{?­¶A"0Â<?ވ¸*º?®uaZ`²?æB+zq?«UA\Èì¸?פ&¿²C:?­ÈØÇn4FGL J1538.9+0425¿À)É¿žˆc@F
;:iÀ:Àß}©yÀ<dQüLY@E…x2Â@äG<Õs?Æ1'®ñp?·ßj‰5É?ððhGçö@(U+«u¿ïá) ¸FÙ?ïÓô©Š¨e¿àò¿¥œÝ¿êqðdx¿ÐgÔ$¯â±¿ïùÕ^kÆ"UNASNone?î´	Çe?›â¸tÊÞ?s>œYτÊ?pï•ãÕjñ?¢W/¾?šzö8P7?ï^¡£õo}?&¼¹æJ?QÙ̄ ٍ?\žKZ_tÁ?".¹É?Ž½c.<ú`?íâK¡,?˜Á*=yv{?'ΠÐÚyç?…øC´,Ñù?²ÅErüX!?""fB"°?¹OÏ?‹Ã&ò—«?¶Îšì?u_蛻§ø?£î!m8Ϩ?ˆÄ:o{n¶4FGL J1539.1+1008?á3"ä}åÖ@G†Ð'}kfÀ:Ÿ9&A³À<WÛçl@3¡B/z@ÙÓËď?Å5 ÝD?±M…C÷&?èh¦è6µŸ?õËÂƹU?ïÿéà
v¿æùÕ
ãîR¿ëË>øcSŒ¿Ø7ÑþdõM¿çdßI® ¿ïÿæŸÜ©ºUNASNone?ï)R	AÔb?™§§¼nú?tkª¤âY;?wS}ôQ×z?•ºÔ.ŒÝr?—Xø\èþ?íXëÀvú?­T°ÞBL¥?'G •[B?›f!É ®Ã?°±•©Öñ_?¥FÊIÌE?ìÞQÍq?š=Çíß?'×}êB?ˆñNeÛç?´W²èô?–[œ4û?ë>$Á'æ?¤½|ïà?±ÞáY «ª?ŸÔ–kâM?´/ø¦…!?™ÛØh<¾4FGL J1539.4-3323?ì'U&@1ˆ5ĊßÀ9(¼QT†jÀ<süQ×@ô$ª"N?øÿ0F祥?´þï3Ôî¯?ä']<ñøÖ@+‡_•'Í@æCÍ_CÝ¿ÓVºÂG¹?ïùgÁf?¾"–}/€¡¿ß';#l–¬¿íH>]2àþ¿ïéŸ
ç»UNASNone3FGL J1539.2-3324?†ytƒ]µ5?ìßZÁ?ïp9û—¨
?ž/mn¤¡?zð-p>?À"Ö\¹7?"ï×%j¿b?±:‰˜)ÌË?íâCPB?½Úy¤Â¢?§ãähFwF?³Ðv|ÛÓö?¥œ"òÒJ"?˜üyÒ?ëµPz7××?¤iӜš¹l?·‡1´Ø? º'ˆœ+'?c<^Òÿ7?X#áEÆw\?îŒõ5¼f6?—
ïöþ†@?¥üëLl¦?–C<•¹^4FGL J1541.2-5201?湫–àña@rkݞ¬(À:×t¼j~úÀ<"K<¤@"QÂ$}@o$ù´Œ?Ög½ž±†u?ïÿV¢N@
ï×hE@ÀUE+Ù"?ïñ¦ ¿ç¿ì3	ý¯Ã¨¿À'åbšÔØ¿áäñ`®—¿î0¡™¹¿ÏèŸ{°ÐmUNASNone?Êó—íh?½¤JmÖ^F?Êú`^"D?ÀŒëê¬?℣Â|)ã?ÅIþa#º?Â9ÅŠš×?ÅN÷ã.ö?Ó±ƒâ™ž¶?Í­¨½Rì?á˜ÌÊЉï?ÍÔºXþÏh?à}‰]tÑ1?°ã£A2û?ÊRX,3+H?¬åÂÎw¬?ÑÛÁ.üÇù?©2•¼bóM?Ås y¸¸?®ç8²m«?â1ªþZ?À)%Ìò?Ñðsžn¦?ºL=e¿»4FGL J1542.1-5901¿ïZ¤˜?XÀÙÖ»cýÀ9H.Ä8©•À:èºÃµÌÖ@…‡°@ìJÆͯK?Äwøõt¶¶?ÂXȃ'ðX?þcˆÕü÷?û")ÿ°z¿à¢R‡"Ä?ïÿRü&V¬¿æÆ×Tæb¿ë®\Ÿ=H¿îÏp;Ñg?ÝßNdgÌUNASNone3FGL J1542.4-5911?ʛñzõî?Àaü$?¦®Qᇙ?¬DóÎ\¸À?çîƒ*
ç?ÂϒíÉI?ěͪEÚý?¾î èZ?²ƒ€ˆØ§…?´,°-
i?舜"StP?Ãw£ì?Ë`ò5›ð?¦ÅZ4Äè©?¿Ìú(i_=?¡×Êú–¯
?å.$-‹m?«
Kî
rz?Á…åcUÍ?£cçQÕ|Î?ÆD"Úk&?­Àpkê"?浝0Ä?±¬Í4Q¶,4FGL J1543.1+4209?¹N÷­Č@J1a¡Û‡À;s¤ÎóÀ<ݜûMé˜@ .ÝNûÖ?ý¼\!iT?Ïíþ÷ÂD?ÌqG€r+A?ý™s,Û@	¸vk5X¿åõí!Öê]?í¦¡‡N¾?çV)Ø@ž¿ãh³¦Äz¿Ú®ÏÁsÓ6¿äÁœýýtUNASNone?ïˆèzåS?˜ãôYvó?^Þ6‰Û?iG¸+è(á?‰êužJœ?–o_³B?ïz Räæ?"'dgà?Nxðÿ>žÑ?cƒÇ?àÏ»?xÛRܑ?'¾	ŠÔ¤?íä°:ºÄ3?™†±¯)̤?}œ÷¸Ë?s\7Îá?®y•s…¼?˜ÇW¼¿Ã?ï™&`¾L?v¼*—Òö?X"B¸?Vãf¦ªæ?†µÅëh) ?u.)'|jç4FGL J1543.4-5925¿îx(]lAÈÀ3ý»'!®À:žlwø_"À;°ñ~\ý1@hwê@$9Ãp,¹?ß#v\}¯X?æQ­Dq@•%t-Ï?ûÍ%7G?ïùrz(¿íUâ_±?€ó;#Ë¿ãéošÂŽ…¿ïýn?΢¿Ý
v[Q	ˆUNASNone?Ä#&‰?½'rÄÁQ÷?¨6ōh!b?¬¼¶¿‹+Á?és¬aß÷?ÀðôqYès?Ã|Ày¸þ?Àø¾Ø ×?§‰ˆŠœ,?®ºàä3 ?é¨bÈçþ?À´5w:©Å?ÕcˆeôVô?¬ºLéBH?Ê3ÎM¿»?©'p	®CN?݂s+ˊ?­GîӋ-³?¶ŸXÒÛ¥·?œxÙ	ui?°¤p²pïÅ?¦>v7Ò?ë†ÏVmP?¬G®
®p4FGL J1543.6-0244¿âªÄä÷ƒ@Cqà?pXÀ9òµ™ªaÀ<(P!Ô@$o¹Ì?@¥zxl"?ÂCK¯*ûV?Ûè]»Vƒ@`ûH
?önrtÈû¿á¤þ§R?ێÆ!7S¿áâP>ܵ¿éšïª/>¿î±±RóÂÛ¿ïÿ"	¶UNASNone3FGL J1543.5-0244?«'GDæÑ?¦GSËQZ~?å|ZèæÂC?Èõ Ý5ÏÀ?ѕE²>¡?Ɯ2í@*?¦ðÿSó?¨vFd?ì»{`c\Z?³Œ}öjoÛ?­WJ¦ÃGW?¦."½…é†?¼Î.Žâß?ŸÂ¬ôô}?å( ©Kb?±VÕ%÷ž¨?ÍRšfa?¬@Ðx´?´), ‰?•N
fÍJ?悤¿B¾?²èÅ£{?Ë´Þî^·R?®sÝ_çÂ4FGL J1544.2-2554?åã)ÒÙ£—@6š€JœÜÀ9žµŒ>gDÀ<n5gÀÙ@"áÊà¹i@ÁµQà?»ï¨ïÍÙ?Øçz"0¤@ëOKD¢@Çÿ_¿ÛÒæÂAX¿Ô³7¥]È¿à`W=Ôvå¿è½¢B4­Ý¿íEK-û»Î¿ðUNASNone3FGL J1544.1-2555?¦¹gp›Ë]?£!±'ïd?쫧:D?³Œn@¹Ú?®•ðe?©§(kj?¹/&V-?¸7
ƒ­?ê[w^aìu?À'¾`v?´æ`F-?­…Ÿ·)
?®)j+kˆÙ?™óýüü€î?ênK9á?¨Mï:—·S?ÀìI6F?¢M­‰"|?яãg\?©H"uæÇ?ܚUÓ
?²Q"ýpñ?Ñր¢IŽ…?ª™'§HL4FGL J1544.9+3218?҇ŒËCÏ|@JÖÜGªÀ;Am
ÅUàÀ<Ç+w}@ ʛþ"Û!@%¸Që…?ÀˆÔº××ÿ³,†›»ý?ñ4XÖZë@ìU¿û??ïÿ?{@?¿íRŠ±ŸIÝ¿×M,Ù|Þ¿ßÖïEG²Ç¿Ê±"øu7¿æÒÎ8ݗUNASNone?îïÊfÃ;?Ÿ™]pËÎÛ?fé˜B"Œ?`P|ÅÆö0?Ÿ)€LG?ž¶K¸…?îìM,º¹²?žÍFåÛÜ?aA.ÿþu?p¸ýz¸³? )é!ddö?œ2ò¤ÈÍ9?íŒ|L¿?–Áëoïš2?tˆTv–?d2WP3!L?²SŸ@WȦ?•ôºU2ÔC?틊Ďe^?™Ž™ÛBÆ?{ý'ÞÛ©<?rôcrNæ?±ãнŸ}?™a'¤¿"Ú4FGL J1545.2-4553?Ô¤³ã
À'@O¿ZôBÀ9òóĈ[À;{<¤ËüÃ@U}£ôC@‹Äߘl?È9…‡¾Ð¶?Ԓ±êˆ@	¹JÚåª?ö³:9·±³?ï½!~TÛgå!I¿çši£1Èпå³À¶‰?¿ïþñ­VåÀ¿ïÔ'£]éUNASNone?Ëþ°™õ-?½ÓèùTiã?šli¾Ù?ºoõÁ#è0?äYã9iÌo?ÄJOA?´}<¦úD4?²¸J"é3U?Ö.ÁW–ŠR?É,"ÕÄâ
?âX÷¿UrP?Ç•ÛtÑ?Ïh%çµå?§æHõS«'?ÆO¦°%?¤šV!…Ì?âžâœŽ}?­F¿"m?©Çԕo?ˆF&6\*?ßYZ±ñ¦?±ºäjþêÇ?Ýncs{­?°ê¶ˆÎ"4FGL J1545.5+2839¿¾G;]5@IÜ1&éxÕÀ<£3vOÀ=Ñö®H@¾d`QÏV@ª×DÁ?ÙfÀ=ó*°?ïÿøÞ£Žæ@
š;e0ÜA@®ˆ7q†U?иw?Ò}ç?ïÿÁeÖt?´Â9JúO¿ì†×6&-¿ïú™Ž±ß¿ïÿý±q&´UNASNone?é(™we†Í?Æ hR~p?ÄpÀ·—?ÃPæ"ãùÂ?«¶e†Ë@Ö?·6,'?ÔîÄ°§ü-?ÍãøiØæ?àÛL9?Ðùg•Ø@?¶an¯¢Á?·Ò÷–ÁaS?áÞFf:Ž?³F§n~~?Ï߀gÁ?²B<'¬[?ȧ#æþV?¥ù®Ó'W??Ў棌?¸S­ŠÉ	C?杵.³ò?»cerwÁ?¥È5îï¤{?Ÿ*ù‰ÔØ4FGL J1546.8-3244?×}´†YöÁ@1¢ß"xîÀ:ÀoB­úzÀ<m¿Ü#å@ r"õ@ÓðØï?€"º•Ë?«éÃþr`?ì8é‹It¾@+2ËÚ3"?²b× ôÓb?ïöѵ(k¿Û_9áÎÅ¿å¡Äÿú¢¿à¬Ô>±·¿ÚàÏ6iIUNASNone?ïAۜš[–?f!™(€?gÅ1Mo?c§ðµƒ?"Ëé&ŠìÏ?91ãMf?ï˜0,W¸?ˆÀ3G?F¶­¨\?VXò?ˆ'ù@.n?†¹D'ãé?î'
ˆÌü?Š°ëĊ,€?uâýRoˆ?lÛʦž?¤"ÇÔu?;?ˆ¶£ÏKÀ?îê(Ѻo?wîF",Â?vóÀä¿9?f³¾¦ã,ù?œþ¡'X?€‰Í^ÁÚ4FGL J1547.4-4802¿äÿëBâ0j@o'½†,À9 MÞ°$ À;lÀh:{ý@+Ý~uÒ@ø1jWX?Ã=ÛØ®Wl?Ә•=×@äZÏYo?ÿlå#/Úä¿Ö#fmG¿á'u=™¾ƒ¿ç|OÁß3¿æN-Š|Æ$¿ïþè=k›Z¿ÀsiN¿UNASNone?½~Ÿ\þ–B?¯Øµ‰??É)^ËÊ13?¼&ˆÂäo?æÔam ê?ÀÔiŒà?À¡'…fø?·ëY`Q¬`?ÔѳŠÒ|?ŏæ¬@?ánÜvu¤?Å*Ó ¥\	?ːª9–?¨-%ÉVP?ÈosŠg?¦š˜ÛŒòV?ã"2õ×Ô?¯ë֒VÌ-?Á£{íå›ø?ž`	—6B?Ìé0° Ÿ?«f	M}q?ä\ÔØ^q;?­þюG4FGL J1547.5-5130¿Ñê¡üax@÷RØҕÀ9C»€t.¦À:æ]	A@»¤"ÈŸA@ãO%AI?À8›Ñr?uကFv?¾=îß,‡?þ"jCk?ïþ•1U¢¿åX5`´ö—¿ë	¯Á¤$¸¿ÛŒ\å^>$¿ä8z?Œ1ý¿æ'zç&ë&UNASNone?ƬDWü9?½?,BXŒ™?‹!œÝ-#?…͉ô,J?éèhw½}	?¾BðP3?ÔyÍîòi?ÅËQ''[A?šz8×E6{?¥hO0Öûf?äïGAÌƘ?ÆT	|­l?Уù$	fX?¬Æހ¯f?­E>œ :-?b+™©áÕ?åÙ¯"9I1?¬Íá
5~;?Éøjµ+ÙÅ?ª!"áY3?Ÿ/3ÞNÕ?"69M¸Ž?èˆk³Â™?«Q¸™Ý4FGL J1547.9+0445?íÛhý«£@E5@N¤©À:ôéË
TîÀ<K¢î¬ñe@頚¿´`@½¶°_¯?Î˔¨î÷?{þì.¼Öà?¯ ^¶ï–?ýŒ Ãås?ïl….¨‰÷¿ÛÜŸBÑ¿á‹Çêüó¿á­.l$‰¿ä¢àj8'þ¿áB£þøCUNASNone?îµ,»ã?ä(µmÊE?`Î÷ûä›?Y?"vŒí¤?£ HdƒE?
TÌӝ?šk±ì?šø>Way?fëÒ»s[?mÞbÿ'?¢×)-«'?™p3)óVw?ìþ/ÅǏ?š4'Uí¼ÿ?†Ç^:¹G?v\ÑÁËPs?µ5¦Î
ld?—Ó•Ž=k*?ëóÿ8dÄ?šÏ†'R?‰t"Ó ö?w³,ævÊ?½1…ÓÂeÄ?™•Œ­r"4FGL J1548.1-4416?ïŠp1sóö@Þá"Å&æÀ:‡0áI\À;Ã?¼®q˜@ËT‹rj@å"Ùîô??ÈýGéΐF?á]ŸîGq@Mý&0ì1@)ÓøEÃ?ìr>
þ¿ã
n}Œ¿âÅ~ú±âf¿ê "Êý¿´¿ï÷2œ4~¿ï 0âvdUNASNone?Ã^|Œ(õm?´ú3¸ïî?Û6ýe?Ç1j·Ñãé?Û2®ƒê‡å?ń_úü?» Oˆß?¼U61ÿ¼=?Ý8s¾¯¦ó?Ê+BÊ·tŸ?Ûÿˆ@<vÖ?Èñ}¶-~û?Ț¿|ž?¦Ò¸Ÿ?ڜºªÏ?µLϘÄhX?ÙÒaå–á?²UÎ8Ñ,?´˜-ƒ6LA?'_@™z9¯?á]á#µ?°–Cs»T?Øm\ë´?®ü"²(4FGL J1548.3-2411?׸ߗL.Ï@7DIDíoÛÀ:†Ôt`úíÀ;ú—t%kÊ@·É³å±@"º\‡À?ÒE3{W3?Ì
/Ä=Ý?øÌs@i|›@j£·Õš¿ìFX^»Í ?íªü-¨…¿ãçŠ$Óõ¿çP tοê%~>Ê@+¿ïû?ÏLÚUNASNone?ç^ÓÿÔ?¿tž«)¦Ø?±×{^¾¡?§LáqÚñ?ÊÊÇ¢§è?¼¾×ia`?€Â8? AŸðYø?|-N>"å?ƒæ>th{Ü?£o.@!Y6?šÁ‰ÞžÛ?æñRÌ??­´ñÿÀðl?´~h«t'?€ãÎÄ!R?Éû©LyIT?¦ÐëÊÒíu?ê‡mV
Ñ? ÄQ¹¥Å:?šV¡âb—?†¹‡ÙªgÁ?_ÑO|j?Ÿ$rYÉ@4FGL J1550.4-5354c?èU¿Xß®ë?ÌRó—罿À8}N€ÌCÀ9ú&	Ã@τ'Û9@ÊÄç%>?Ûqšânõ?Ì
>ðÛu@1bBë7@m%-O™?ïþ˜½?;?"¼ñ@'@¿èÇÚÄç%¿êë)CÆ(n¿àÞLÑë¿çÓÀì÷UNASNone<?ėµÙ+¤d?ÀJ®0?Àʎ J;?Ö´Gk]S?æ§o¢v˜?ɃQ1É?¥&RÉ	['?¤Gd[
dP?±ä8ôС?´‹ì'Î?쉞LPÐ2?·QeÍî"?¸ŽVÞV?›&¦Ñ=
?ÅYŸ¢G®?°ìd+å?ç¦L'pT?°¥¥>ÊÙ?›Uîn϶?""œœÙ"?›2yŠ¢LŠ?•!℺I?îK¼À:??—ýÍ·74FGL J1550.6+6027?æÔJUÊÉ@F‰"_ôöÀ:é5WСnÀ<ÒÝnÛî@ q¿ºëxß@³Y¼3øU?»__(R/¿³è‡UYh?ôý7Σg@¡Ë:¦o¿çxÂ
?©¢í\M¿ç›8 Z}û¿ÊžI—"ÆÔ¿ádãD–Í¿Ú4Ci\UUNASNone3FGL J1550.4+6027?ï¹ÝÉmš? nrٕb?LÓØn<"?O´¿[i¨?v¹7»k…? —´R¤í ?.ƒ5'?†U4ïš
?BÑø¡>·‹?QË%"3§™?…éÕ¯ì?…4š'o/?îáuÄå
?†Òß鳈Ò?f¾uLêEº?W«§r? |Èã?†ú9PÒ3?ïw«`¨ö†?w#¦ÑaN?q^Aހè)?a5ÈØКû?‰fæêt?vBån´4FGL J1551.3-4920¿ë1ò_8N@
x¡Ú°»À9҃pbh«À;/Ÿ(NÓ£@s˜.4›¾@P¤þQª?Í×yär…Ù?ÁNÔäÉBÕ?ô…Őe?ûÍQ¤ãNÄ?ïøM·†ê¿Þ3LÉn¯¿êâѼÖ_¿âhá}V¿ïø¸BÒ¨?ïtã׫MUNASNone?ÜÕmžË-?ÅéuÈ'E?Žn±cðN?ŒG=])Êá?á}+Žk
¨?ÆI։›ó?×øTò-J?ÊáÚzéT|?°£œ…Ÿ/?´£>Ü?ù²?â aö5u?ÊD¹îɓ<?×0"ÑÞ?°.0T	œ?´¹õ"?"ô-Mx:g?áö©¤°?°ú@r
?и?PÀ­?´:÷{}æÞ?¥ºšOÎM?'ÔrpDÛ?æHFÀ¢Å?µ¢ß9‹ÂÁ4FGL J1551.7-4257?§ÅÊÁX5@!*2	g‡ÏÀ9ԗt%kÊÀ;‹Ûz¹×@ššÊA¥@Úú—
s?Ãóâû¸G°?¸¹Š¿zîx?ô,byqÛå@ªëhÄ9«¿è4ÛϲZ¿áâ~
ÇÚ¿éGimO¿åÕ¥¹b¿å"&"À¿ïÿÀ	oëJUNASNone?ãµòØ9ðã?Âθš:3?†¦þb?€%JHã˜?×ߢN¦æG?ÂÏMçP?èÖcâ?ÆTZj¾&x?ˆJ!
Vô?'—4%˜˜q?Ë!Ѳ×b?ů7"¬ˆ?âc,\Ø-?±w0ð¸bG?«½&ÆðÇÑ?'t{ê\Kn?×ÂVÎh6¬?°Aå&™'?èµ$ð<Ýo?¦`=ړÏ?"—Á9JB?{ÜY4å?ʳFå`ü?¥ó$
'ÓO4FGL J1551.9-6015¿ïÿZ¬QŠÀÀYÓpóˆÀ:lù¹"á¤À<
øç
¶@š>C\¡@÷ÀOæÈ?ÔðÍÝîÞ?ïÿÿÃw@zæ ³iN@Þȇî¡^?ïôž"|å?Æö©j(€¿éo`
+Òí¿ïôQ«Ä>‰?é©£½^ð¦¿íMt']è¾UNASNone?ã嵶ۘö?ÊI%?¢Ú™?οö
ë@§?ŒK¯hüÅ?Á©3¦[?¿œÝ'UÑ?Î+þÚš?ÈŠñp?´vôÎúþl?À=ÜRÉi3?åêÖfj?ÊlÔ®Í?ÛðCÒqNh?²tïå?ÑÕpZ?°¾	&4[?Òú«¹A=?« S1?Ý1Û ôkð?ÅѯÉ­ë?É	}BQF?ÈbÑàÑbS?ÖB  jkn?Äqv\Ák4FGL J1553.8-5325e?ōÃ[?Ñ×r"eÀ6ˆËà=ÂÙÀ9‡‰Fe?@i9È£T@EüÁ‡m?ŸÊ
ª¸?»Q†'_8@¢l] l‡@©Ç "?ïÿÑa\w¿É_·
BÏ¿à-â@ÒX'¿âl"þª?"¿äžJÞÿâ-iànjAUNASNone3FGL J1554.4-5315c? W‡ïÛý?±7šß?iñRß ?{àõ}:?îàñ3¯`?±°óĺ¡?'
¦…Îę?œÔO7ñ-?Ù}–"L?Ð~}¸6Ô¦?â¹€‡ãÓ?Ðb¯JÚւ?²-Y~<å¦?žè+àWjý?¶%þǎ—Å?¡‰"#w?êõ"÷FR?§ç¥ôs
·?rªžÍ?c6:nX—?À¼l^Ým?­Z½QÁË?묿"'g%?®!*@HÇ24FGL J1554.2+2008¿áÿ/ÞȀ@Gäñ<îØÀ:³È±µRÀ<x úK‹@!x?×±W?ûQ¦&oÖ?ÁÆ£}sY?·KWí&ßh?÷zÀûÞ2P@I*-¦…¿ïÙ	Y¿ï@…3Ç-?ïùV˜"	]¿Õ\…ýZ‰8¿è•övêB)?ΗådsGUNASNone3FGL J1554.4+2010?ïž‹úö#?'F;"ª,!?R@6sW!?O5"_žÀð?†6V2ד?Q¡±¨º\?î°$Ùx?¤÷SÍ2Üã?k¡Uëêð…?vÛ¡˜*¢L?£C©±'?£Ìús3t5?íÅ 6JÂ
?'Ä b''?zsäg‰Ï?p,ë''Òú?°+Îcw?¨m¿gÕ?ì>Yä=-:?£&C«?ƒ{f™€ë?h!¥zŽL?»Ä
æxÉ?¢l³8¹
4FGL J1555.2+7103?ÅÕM™@Cš+<¼IÀ;
iŽÀ<å4W¡†@sgÇ9ï?þJÀ¾¡'?Òà!1H?ÞG^á™@h%ç}R?ý2xUQ@:¿ë64¥#:˜¿Ðô!:kH¿Þ¯_ÑvÖ¿åÑva†-¿ì´
(wîN¿ïüP}ÆÕ<UNASNone?답ªæ$6?±ÍësÔ ?­}Õȋ?¢Ô±Æ‰q)?µ"½ê˜Ë?ªñ…í/µl?çæ=št'?Á0…¨$×?¼þåí‹2{?¹µ‡LלE?Á瘖Дº?²ÆA	Šk€?ç‹ßQÌgþ?«Ñ‹L*Öì?»Ô××#JØ? qÚnG­©?ÃæÍ<º¡?£øýSâ¯Â?ç䤐ö,)?¬QšTÝW?½T÷ß}Œa?¦Ö†W#Q?ÁÂñÌh‰-?¤D—þOßÎ4FGL J1556.4-6911¿å]¬R¦7"À'öº «qÀ:¶"ÿ®¡iÀ<qzØ
r¯@28EìžN@ðüõŠ?ÏcæÄŗN?ÙÙØN
O@¦ÝA‰?üŒcXÊÇ?Õ%ðál—?ïâàj8'þ¿Þ•¨sQ0t¿Úf('íמ 'ñ¿Ô×[œãUNASNone?á|†Ý}´?ş#xÔ´¹?½äHÝcI?²êGí\TD?Öeô»ëÇ?ÅWr>.Ò{?ä^³=4Ï¢?Çѹ<2s?ÇСS)o?Á÷psù¶?Æ´'٘?À§êƒécÎ?傐M½:d?¯M¨úÄ¿?¿UÜÌSœ?¡"}¶†£?ÊJÐbዣ?¨¼/Gƒ@>?àïù¯=Y0?®õlž.bö?Ñ
Íï¼?°n¢Œ¬?Ê*7+#
?¥ö
-Õ­4FGL J1556.8-5242c¿âú
·WßT?áG›*½™À8ÐÎ{ùu¢À:Qqâ›k@ž>õ3HW@ ~ÅؼÅ?ÍÅrûË
?ÖZÚÂïI@
Ødà
—?ü…¤DBz?ïó…hŠ-¿á{%oü^¿äÇ QºÞ¿éÓ¡Ó#ÿ¿ëTu£KÜ¿ïÝ{¦i‹µUNASNone=?xkßRÿé?wNbx‡Ñ?‡	r{;·? ;; +'?ïsïÕ? ¿à!æj?™fò'¬Ú?Ÿñ«ç}þ?®©'©ý¨?¯÷›AÔ?íJ/D"¾§?±­åq"^P?³o8àw?'qh¶f?ÀŸLéE
I?Å†ñ†º?éj<ž'­½?¢R!Ç?qP¥3ö‡?`)!kBœ?­SƔ{à%?"\Ùg4©?î¸õmÚ?•B=zA+4FGL J1557.2+3822¿b[-ÎÉiÿ@HåæFñVÀ;ôÅjüZÀ=ž¬(—@ TÜY×`?ýZ&6Ën(?Ö6ë¤~O?ËÍ&#€7É?õ	:q@ÿxÍFD]?í :}Ti?Ô¢˜[V¿âå¹ÏD¿¹u‰€-+¿êÇøð?ŠÈ-UΓ¡UNASNone?îL¯pRÒ?¢˜Z9'¹d?…ûn¿s?'UžeÓÅ?¥¶-q
#?¡=՗^¾"?îí¥"•5ý?™–Ìxò¸¼?ewNX>ת?pV¥×[«$?ŸœqâQeX?—{¤3¶ÜT?ìÅ´Äv}?›º¼vôà?–­&d82=?‡¥ßÅ|ëÍ?´8ˆÀÎ?}?•Î÷"Ôd1?î"$÷°·‹?Qþî®Ñï?"?å:o8?yP…gr8m?¢­·6XÅþ?ŽòO¯)4FGL J1559.7-4518?݆>sV@nžÂÎFJÀ9¡Ä©èœ6À;ULf
 @¬3*úª@°#¾…â?ŹxǑúi?ŜçAm2³@ÅáõRþ?ù¢¾Úzà¿ìZÓÍ$á¿Ïߒâ›@8¿åÕí¨§c¿æÈÙ"E¥¿ìEÞ,ñ{¿ïúÿ?8$UNASNone?Åâ|³o˜?´¦0}'å!?¤äU2f? ‹¶ò]ª?é9¡1?·«Q(À?É­é;L;ž?½bit:Ð?Á]~ˆPâ?¼•Ï r‡ü?å=&¸y?ÂUhf–`?ÕÈáÊøY?¯'–/ty?¹sד¼?˜dªhhÖï?áí("¼?¯U÷žWŽ?Ñ
`¤G?ª¥Î7ˆ?¾û[6ãe?¢Zb_>hì?ãši41q?°=×è2P4FGL J1600.4+0407¿Ôk=RhO@C¸ƒBÙÀ;	ð€0<À<€Ü…§tN@rX¡×«£?ÿd¢¬gÒw?Ïe»d°?ÈPIÄo0:?ùꁘñÓí@+´Ýí±t¿í‰Ú¿~°Š?ïÿVW$ª¿Ëú|]s¤¿Ú—8Á< Å¿ïÿÇËÜ?ïýjŸ>XUNASNone?ïaSl1?‹bäüãë?s©?Ïuz
?t2ø°õp?äË=!6¿?‡;¡¥"°?ï<€h˜Ó?—=ç†?`ÅÓ|ú$P?pÀ'ªŸÚ?–NõƒM¡	?"ð`ÿVô?ír¨àyˆ5?–qØ^?"Æ "`©B?ˆ+¯OgôM?®òaç7(?'3d#,ð?î©s5íí‰?‹ŠFú ?z¨Cé8/¨?mjŒ2óÑ?¢Ä#ú!j?‰üT'ßM4FGL J1602.0-4402¿ãÞ
yxr@-Õ
ˆïþÀ9Ú|#g
UÀ;h¦Bˆ@§*ѺÈ@_tÝÛ?Ã|(ÚêœÁ?—Ì—ó§,)?Ùhm
&Ú@úã(-ñ€?ïÒ6™A¿áÂlÁÊ:K¿ìY …F%¿ÓÐ.`æt¿¿êŠ?åHD¿å³JEžpUNASNone?áåêɄõ?Ǧzr§Ú?'>p/ko?9‡×2(H?Û¢8O»z¼?ǘ5õ2î€?æ_†nÂaC?ÄAw/¼P?sòo]èÙÉ?Šy/­?Òñ)eš?Äwª…B?æ[6I«ìÃ?²HµmI?œ£ÝC—ª^?‰û¹ÿH²¤?ÑU˜n«Ó?°Üˆ™Ùé?è=¥a?©¡ËKŠá€?ˆ"1|­Ôu?sÿÕvMÒ?̀8—½3?©YÒ€3l4FGL J1602.2+2305?åE8ãe.r@GoîN&ԀÀ:ß­z!.À<¯-‹S…¹@7ö'lO?ú½S,;d?ÌE}x%Ö~?åN•ÄøÂõ@˜u—5@ Žˆny?îE6̤¿é'ص8['?·SëåkÕ¿áçÁŲ§¿íB8¿d.~¿ïᐼ{UNASNone3FGL J1601.9+2306?±ÂÊà‡?°Ã–¬ҍ?ìA‹)èl?·f'9äp`?¨a·¡xý?«ñ:ç­7±?»›R­_<?¼»Ú™xõ?鳃¬ÍѼ?Ä4¸÷±i?¶Èäá?²ôjÔýPn?čÐX™é˜?¦V'äʶ?æ<HÄÈS[?®…ÂÁ6ãµ?"DÈü?¥uaéík]?ÏB‡ÁÃk–?¯"5w|c˜?á2רGÝÆ?¸½f"¯"?ËòT?­{ixº?ü4FGL J1603.0-4808?î&q26!ê@
ႁOùÀ9bžÕB½À:êæ0K!g@ìfOë$Ò@¿ãzŽ;˜?ÒLóc9‹<?Ôâ¿ù&È@Ù
By!T?ö>~À¨?ïûüР–ä¿âÝ|²ÙÀ¿éåïaLK¿è8«bnà¿íxrmæ¿~­C¼å›UNASNone?Ù3ÀûòW©?ű¿(îï?ÅišáïV7?"本ɒ?Üq"ý;?ǞՍá$?Â,܅3?¾Ý¶¿ƒ9Ë?ЩV†Jˆ+?ǯ3ãt~N?ã(I¸cšž?Ȳ÷ß)?ÊÇjgw"?¦yéMõ³Á?Dz»øè8?¯I~ó¢?ãavb!è?±à_×ÇLÞ?©æ>ºwò‰?ŒþÏrò0j?ÍZš.yu?±ðt!M?çmÌâz?°Ñ/#­´m4FGL J1603.3-6010¿ÚNA‹)ƒ À̎ï¬.À9Í,Ñb¨À;ÿV?§µ¼@+~d	û?ýù™cé´d?ÁeFc¡?ÔÓXl¨ŸÇ@Ëï»@öצÅ|!?ïõ(5©/9¿}-©Ë.ÖÇ¿Ùä½ú¢É¿Úu»Ÿíq¿éõH·(ö™¿ë½¢yMUNASNone3FGL J1603.7-6011?°¹-¿5?¡µëÊ`ê˜?âXñï@á×?ÅÆا G@?×б¼ï?Ãý#!Ä?·®?É,è?³ykƘ?×ÌÇðü?É¥1Ê!‰I?á˜4"áå?ɐRéf®Ì?ÉÄõ
tèô?«n	šÒ	?áÌa–ƒT?³îÓÝÓ?Ï	†·1	½?ªoSrt?ÐÆF®ÜÍ?¢ÏF|¾ŽÃ?Ó¡OX÷?­¸®E~Á†?ۘ1ù=?­áB^…ó4FGL J1603.6-0451?ìóþBÌ¿r@@ÒÒ¡øã¬À:<‰œÌTÀ<
Ê©Üݼ@3»QzF@ÆH@áqŸ?Å|ˆÑm?¸­z÷íâÇ?ò9,qx@fº¾'â?ҋ¢cAÄ¿ä'|^ö/¿ä‰}+¤É¿æ•ò—Ÿï¿èÒŠÝ>4¿ïýýâŽlUNASNone?éõgYü¨6?¶­C-€¼ü?˜îÚ©×?Œê>½¤?Å&äÔ2	î?¶rå=¤Ï?î'þ%$v˜?›#û㕳?uý®Êöú?y]ûjîQ?¤-]÷ß7¤?˜–|Ñ3>?ê|¼?fh?¦4êêH'?¢|ê¤ä°?ïoxÿò?Ápº™-0?¢G*¿hØ?ëÝ#-?š¦*á0¨?ŸRl?$•Ú?'Ôö9Á"Ã?À<{¾à?˜jÜ '£4FGL J1604.4-4927?à#‰A)7~@Àù²%À9:×ÑÍnÀ:¡²okÉ@18qÜf@26~AN?É
¢Gèø?Ӑ±þë-
@gȖÝ@=¨ø1TŒ?ïáâ"o?îƦ!è2.¿ãZ-þ•ò›¿èòbüO¿íRC™²Ä
¿ïýÚá¸lCUNASNone?ÓÅ÷'´!?ÂËÎb£éC?Ëg{­ç¶?Â,vAíj?ކJätë%?Ç´Ô÷#œ?Å% ?¦0‹?Å>•ª…l?Ð	é5¾r?Ê=«ˆr?â²{{"¤?̓ãzh?Ï&ú\˜?­2ìЙo?Ä>ÔyÉ°?¥]ŒSàE ?ã)AZ;¶o?°NÓ[ÅK?µdΠ´Jð?œ;E¦]Ã#?ÇEû°˜‡?¯k"û†%?ç',ýP€?°ë©N
Jj4FGL J1606.2-4602?¹%ˆP3-±@7 ÜïYÀÀ9üÒhAÀ;'²køvŸ@‡,ÓH@éi]'¬?×s]á~?ïÿ®2D¡@öà鳍@˗P=Ê?ïäžvx¿Ú'¿ó v¿é¥ø']<ò¿ïÿB€X*¿èt—1š­¿éØAŠäËUNASNone	?àoà,E}D?Éáô	¼#:?с•Ýe3?È|5g~?Ë=S"µ@‹?Ãx|‹I?µÂ1Œx&	?¸žÀúH?ßZ÷ÈDôç?Ï^%ù ?Û4{ԝ—?Ë£q·&¸?ÑÉï=CX?¬·?ªuH?ÎËøeʲ%?±°"ùáˆÔ?ÞÐîÝÝc–?²—}‡\Õ?–ûRŒFt;?†î1pãj?å}kWC:
?¿Ï"TE>µ?ӕt(µ$¦?¾Pq9ߤ4FGL J1608.4+0055?ï²É24@Bà~ZxòÀ:"€žP¸À<<g/ºï@lpÕ«Æ@)´Â&?Á">ï)?€» ¹Lé?ÁDŸ—4@Ì}EPC¿¦~ƒœ4Ý
¿áÄÁ/à˜\¿å?ÐÐgŒ¿é-=%$}¿ïˆ3
‡¶?ë2'¸#È\UNASNone?í2½¨+.ì?²Ž81Xå?‹Y+$ȃ9? ]¼ÑOÀ?²þíZ
x8?°¨EŠ¥ò?î×ešZ6?£jª«Ñˆ£?p–%0|€N?zm|w$Óë?¤ÅJ̟?¡ô[o®?ìÐÇóŒú¾?™íRû~üä?•hÕæ…e?"Áړê?´ŠéöÐÇ?"¤@ÁÕ9?í¾D8D™?•§n/?é?ŠOõ\ø?|¿¿±_?­tu*_*?'×"9äv4FGL J1608.8-4803?ìõUš;U@"ÛÄ·UÀ9"¾®&˜À:¸Gõb@ÎfæÀ@—G½-óX@ëMý¹Ô£?ߛ9ÂC†è@ù¾$"]??úܔîZ¿àû	á€8¿ãr;ò•í¿çiŒöóçÄ¿ï8ÜÀ_×?ÕH߂\L¿ïù"–,ýUNASNone2FGL J1610.1-4808?äÅýle°a?͐8Yª0?ÍßV7A±¯?̾ÈF{J¯?¾h.Oš?¿1lˆšsÙ?яà:‡ùw?ԝîóœ?Í{Ÿ!J8?Ô°ýڊ@Ÿ?ß²P4Òþí?ÕwM.´¤?ÉF×Suî¶?¥ã©ÈSCU?ιìÂì=X?´æ!ÂýË?áÿÎúgtü?µ<8Z(Ø?æ
='´D`?Ú/	CTÊ«?‡vPûA6?¶š¬ãO‡Õ?Ó/ÒR½nÝ?Ùèiî;‰4FGL J1609.3-4326¿ì¤r‡ÿ5@c%}h
«À9ËǐíùÀ;[¦?šIÃ@	àÀõ~@ɎSë9Ÿ?øS"¢Ù´?ÚMú^ÖO@ŊžT~@zYWµ¯?ïÕ½Àƒ¿éÄ#°ß0}¿èb­ß¡»§¿çÜ$X¤ÜÄ¿ìFö£–¿—ß~øzòÝUNASNone	?ä§Ê`Y"?ɏãlu¨?Ǥ‰ÏP3?ÇГQÄ«"?żL°:}?¿ô¢°"÷¢?Ùö¶,­?А´nk¨?¿IŠ,P\?Ãn™£	Ÿ?ÞE]çH>Û?Ìßn<
¯©?߈pžá˜²?³ÔU-,'?¿ÅÞjÞ<}?¥ñÊßß?؆ÆfØ.?±s,b½C?äMWr½?Í-¸"<Þ6?†ÌcŠç? } ­»ê?Ö®îß5ƒ?Ìïï}lÙq4FGL J1609.6-4837?ï­ú‡˜@rï
åÀ9Ú'(böÀ:•V|
—˜@wh&"ùú@FxõŽ?Í2×XA	¶?д䣮…@ÆeÊÞ@[¤ÍOA¿ëLA³Ù?ïŸá§Oe¿çì×Ï_ND¿ë%5C®«¿äj)i…Õ—¿ïÿÿÊPËUNASNone?åLjò²—?ÃG
ËgG?±Áöàˆj?±Ã¬Û6N?Ðö¬b"ï²?Âfxñ†îP?Ãj8Þü¸&?Átj*?Ì#ْ`½Ó?ƎYäú?ä{c¨¢?ÊLãx΀?È£C.ãã?¥ŠQÂ%Lá?Å| q­ë}?§™ì»¼Tî?äx'ی_?¬áDzÂ&á?¿ϊ'Ã?¢zœ³æR?¾Oÿˆ'?§³Òº²l'?è\ü¾½w?¯#¾âú4FGL J1610.3-5154c¿Úž—Ùò¿Í@,ÀÓÀ8wSŸºEÀ:óøŠÀ¹@tœ…\JÚ@z–¹ëH¹?Å54?LÇ?×6a7R}@jaâs'?ᝄƒ:'¿îìñe2‰À?ïòË.g˜¿áõ³Á
&¿è§ØVmÊß¿íûW>«6z¿ïüD¿L±‰UNASNone%?¥wJP+{?¿V&zžì?Ëé@ƒqç?ÅV)§¸É]?ç®;::2o?ȨÿÛ¿+!?' ÂK•p(?HÌ/z?ܳ9Û`h?ÎDPã½:º?á[à	!Ÿ
?ÍÕ3¹Fõ`?­ZèéG¼?'¸‡ÁՔ?Ð0¬ØCq?°[®ÇÌ?æ"'ûIÌ?°r4ªtP¼?Bn:€Ÿ1-?25"Èç´?ØDô±M€+?¸ÏXÈ?Ê?ãØê¹?¸'€_Jm4FGL J1611.6-6013?Ó½8Ò{ÛÀ»<ĬlÛÀ:ïÁÄ[À;É°pçÊ@Ö)ax@@•sd{ª›?Ðã`¸vÔ?Ö£²A†24@hXJb?õq	̆+?ïû?¤Á¿ëž'ŒŒÁ¿ÚÝFA­ÊS¿æ¾Q€ž¡¿ëV8!ï¿ïøžý†¨üUNASNone?Åô¶ÿ|¸?·«ïK·Å? 1Çéät?Ÿh«x
ì'?éXµÁ'‹?º9ϕrà[?Ëd)ƒ´®u?ÅÀá|?­ÍCÉåà¼?³~'²æ̘?çJ!btvX?ÆKîQ·<?ל…t*ƒf?®~†i¿k?ÄÓh!w
? Ýsïµ ?ÝùÆ{÷?®E؄…?Ì¥F*Wñ?£U[Þc%?Áãd!ðã\?¤ºtË¿i?ä]ÕlíÊå?¬?AL)ò4FGL J1611.9-5125c?µÜÕB7/¿¢ÀòyÌéÀ8$¹ØÔBÀ9Œûµîcö@xOE¤~@ŠQã!¢è?Âô`$-ó?×ÅäêÑ@"8]>Ÿx@\ÏRc$=¿Ï2¾°Õ?¬£"Šùï¿ãW榒¦`¿é'š¡×U½¿îûs®çŠ¿ïÿcøÍܗUNASNone4?oÑû*èÎ?p»ýOqÊg?Áyäß;Šd?Á·ñgs4?끴Í~?ÁèÈ|?Œv÷;NP?"'…•â¢?Çx}þiq?À—'û¿Îù?éÉF{xj?À‰"@žÑÉ?¤®Ñï̑?ŠÍlãÄ?ӏ¸L.r?µŸÕå'
î?äí:üÉÊ/?µAÿÚ:/?QCmG÷çÃ?B…å–D"?¼«WŽÙ¬û?¤úoŠ~Çÿ?ìaóW€Îm?¥³*Zö¤4FGL J1612.1+1407¿í:åî»,@DÍÇ%ÃÞèÀ:†w-^À<ÂÛpÔ~r@Ü0Âë?ú†ØF}'Ó?ÇëX¦4]?æö·¢CC@¾1)?÷ä‡ÑÆÞ¿ïÿþøþ"?ïÿk»9ýR?»"òm›9¿âòq׳°œ¿ìÐ5½Q.Ç¿ïøœ>9¡ŒUNASNone3FGL J1611.9+1404?°Bá	¢¢™?®@ƒ=ä>	?쒶¨/)?·…м×â
?¦NÓlGÈQ?¬Y)CTT?ž'4ŸzÏE?¦cÊT¹í?íª@$‹?³Hþ£XêM?¦åùè4?¦&y°PÊÀ?¼~	j´fù?¡oÑg<F?èºÂ/µX?¨X+H¬?½±ƒÍî=? žëq'?±¥Ä;›o?›ùÁ9©?ê{±[zz?°cÙ³°Rh?º'&WèÁ?¦upJñ®4FGL J1612.1-4526¿ìªGo]ä@5àqÅ?:À:"Ëùh6JÀ;ffÓs¯û@geÀy,g@Ý`#Up?Ùª\²½­?âH«4̐g@dϝ,@ 4¸ïJP?îÂOpV¿ä?3ÞLQ¿á'ˆô'¿é¹È®Zÿ¿ïý¸AûM¿ä²@Äì-»UNASNone	?Ðì7õ©Å?¿2$ÒNŽK?³DHkí)˜?±vêP†F?å!Z÷­Íì?Á¶·Æw?Ñ]b'sHV?ÅCö÷·Ñ?ÀÒѽÅ?ÀKÍí¿ô?ã͊~¬d?ÆÔzâñ•?ÔØÏ-
2Ï?¯án€c#?ÄV,eׇ ?¥­ bûiø?à~
P"°?±£bìÓX?Èù'òU˜?¥b#ÂÐqÙ?±»,ïµ?Ÿ²}³kÔ¯?çŠ8Ý̹%?«pvút×4FGL J1612.4+0409¿æ·ÿÈøÜ@Bu"úÖËSÀ;Ÿ$`2À<±ÑtÒ9ô@ò§´i??ü¼˜6Ã
¬?϶ÊÂ["¶?Ø×@	,LÄÔ°Ç@+e¢F;?ïæ'j(¿âûjÚim'¿Ü&ŠwÔx¿ÑgïØÓÁ¿í
â18¿ïÿ›÷Aë]UNASNone?ï{B@j?–`Oßö?ŠÀ
r7?…ÂtJ?'p²¹°D?$½M=¼?î²ñ£ÏÊ?¥Ý­Â8Ž?…w™˜úB?Ê Ÿ,¨µ?¨§\ÄË? Ä²"_?ë²ìô¬ž?¢Ã,ñ±ã?¨ƗÝV¤?"Ô͙uxÑ?¶fµ¬`2?™äðeºî?ëtx" ÄÐ?ŸÍŽp¼†?¡`+Bp?°!pfíÐ?»¬%ÅóËÊ?›gbõ4FGL J1612.4-4419¿îzŒåx_@MhÍJ¡À9êIHHn.À;7oE298@×ÆÎ0$5@üa'?ÕГÁ=w…?î÷‡ Q»@ً÷ðg?ü›è~Y!¿ïø罓ô¿?ïï"Áhj£¿ë/¿5_ˆ¿æúÖ?½/K¿Üõ™Ÿ£ÉÉ¿ëþ!²WVUNASNone?Şk—âë¦?Æóe¬e"?ã °k˜¯X?Ö|uL<e0?ÍÞÒ¹ºVø?Îãg¨ø…?±ßòMWùÃ?ÀÈÛj´bï?äãá
)¢?Ò^Ò	ˆ¨0?ÑÀARV½Š?ÏIß\êЎ?ÎÏü€"Œ?§JNå
!?ʓ*ŸŒR"?®£¼öÓT??á§68HV?°'áÔpeu?O­Þe˛¶?e5-1/?îgBäFÃ?·B§G#™?©
B•]?¶ìþQßã4FGL J1613.0-5102?Ý0þ# ²×?½ò6=Ô¢À7Ù¯ÅU	GÀ9Š¦V@~u@ªŠÀbÜ@r.þñG?¾Ì¡Ù¯l?Õb'|ñ˜3@¯ªŠ'¥a@ ¨²fD¿Ò[—?ø¡¿âG¦Ý¤áK¿à—à?ñ2¿è›U%ÌBc¿ìQ'[¶¿ïþ£^"_ôUNASNone?žS}<y?z¸ºy"üc?Ù-L '~"?Ì\¤»G5?ã*H¼Ç–?ÌmhÓiJ?"90–5…?ŸhB»¾J'?Ñ¢i:}<?Ê¥ËØ…?æ•ÞJ™N?ʪ
CÊá?ª~²™ûQ?™¤0å[?ßY܆•ä?¸­ÇW/í?ÝVa㡲?¸\«æé²?ZlڜêÖ?KÞªqÌ×?¸o>k×?¤~±|áçì?ìäáЎ]?¤‡~K/Ð4FGL J1613.1-3840?×íAG¯'\@"$§Ös>¼À:°ðs›OÀ<
N‰Ðκ@ ø*$Á«\?óDJè[žŒ?áŽ-àc­?àÚ;ëh™G?þ1ßÈR@Ž¢ÛÔÊ?çZ,Ñð"<?ïxe!Aï¿ës…hŠ-?²(þ¦ä†¿Þ……zþ£ß¿å̂$2pUNASNone?Þ\!Ù,?ÅþËÕݤU? ™^7"?ž'>"~z?ßÙÅ8ã?ÆYKõ€8¼?ãäZh=÷¼?Ð'Ò?äMD?…\¼ý849?œÛ}>ºàý?׌eGšNç?Ï`î`ö¤?åhÒ&]¹?®Ìp÷R™å?­Ç~äÑlÈ?–T00Æa?ÑukÖEô?«×µQ?éÎ~;Œ›?²$*㮲2?ssp|iŒ?y~p(ä@ç?È-ƒvL
J?²Bpz•0r4FGL J1615.3-1512?ëK¨R¢˜@8è"Ýz™úÀ:ŠŽ]%uÀ</j£	@­w'ÃiL?þ:‹KøüÖ?Òf';‡?Öó{!ßMÙ@f"f\Uk?ÿáJø÷£?æ'$óÅ¿æ´2ÝeK?çè?º*2Ù¿å6<!ÄJó¿âõ@S­&>¿ïþ¿UØUNASNone?ëJ*à¨cÑ?´´ºW½ç3?œðP1DéÈ?—hÛFÔ?¾r"îk§?²D$ßjz¯?í%æšN›Æ?²8¾¶!
Ô?–œÍ"€oj?¥ÛXUbl?±)—Èkø?¦ò­œ"z½?çɌ6¾x5?¬ÉyùÂ`™?±¥ÑG…Ìÿ?™w;ñ§ƒ¡?ÈæC8«?¦mœ¥´"?æöˆÇ|¯?³0¸|苜?Ÿ \Ìýя?—¤ÿœì›,?Ðè¥#)‰?³z¾*'4FGL J1615.5-5434¿ïÄÝ)¼<À¦°'ª¸À9á÷¯îpÀ;Fʨ/^'@Êx‰©@'ì®êc·?Çîüâê?ºd Ïª?ðxºvˆóY?õaDì³r?G)Š=¿éG1b"´á¿ã
'ž*x¿èVlˆ¿VÿáÁ*l»>¿ç+YnLUNASNone?̺ôÝ+'?º˜nXIJ?€x; úÙ(?vŸ¼1Ù?è½0TDÉÒ?ºý?3DP?ÇIӖò?ÁZÓg›W?'ú½Q0¢?šl…"hœ?é©× ¾g?Á)vRÈ-?ÓE'EЎ7?­¦§-.¿?¬¬³hÇO?Œcòû4?ä'k¬Q,p?­4vÛçh›?¸€Vz»Ô?˜áˆIj?¥ÊÁ…}eo?"ÐZKõ_?ë"I$øÒ.? MS-"n4FGL J1615.9-4322¿Â]VG_e@N0DkjÀ:"A±{7¯À;jÃwï%@ÀØ#B$h@8Omü]?ûéM¼KuI?εN+>?úzDºD4@ÜCR:4"?ïb<jêY¦¿ß	?"OZ†¿ë'ñ¡îQØ¿æn~ãµÇ¿Ø°†zØä2¿êƒËf›?ŒUNASNone?É:b5ÑüÅ?½ò°aü?¾›#
U"I?Äç.ùÆG›?åÞà܅?Ç<À§™©w?ÜB<‹³2
?Ð;Í%ît<?«¼×Z;'?¸çïn!œC?à#D'µW?ÍxSÛ?Úvpk	†Q?°¹Y)f¥ã?¸«ç‹Õm? Þ"{Tt?ß^•²3Õ?¯"ÒË×b?èî©ïerP?É'Q§È~?YüÈNuyß?{8æÉé?Ì^±ÍKÍ?É6·Š4FGL J1616.6-5341¿ê@É)1Û"À[!f'À9]ħd]À;Ùô¦/ª@@§.­'@›Ç »aj?À7™NÆ?ïLùx&'K@!Í¥¹bŒ½@Ô+Ž#CÒ?ïäiÁºŸú¿Ýƒÿ°É¿½¼dãoü¿èŽ?{¿î(ÀþãJh¿ïÿUJÃUNASNone3FGL J1616.8-5343?`¥Š«…?`Î0]F~?îñ<™"(b?£t‹P'?ŸÃ»›·þ<?¢ÉO-'½?ÖùMÃK=?Ž:«´i6s?é8RTÑ?Äâ$™½?ÊG‡?Äwêœ.?¢KÀÖC+!?‹Žì —"®?éÿ…î7M®?¨µÞT!ä?Ãnø'þ?¥`v%Øro??'F†™üM?4 \Ö\=p?îÐÒ7
/‰?˜aÎJDR?¢³¸ӈ?˜4£S²Æ{4FGL J1616.6-5009?ïêÃQgÀr?×ٜSˆ=QÀ8LÀ½ÊÑJÀ9ÍLê"]ð@ À‹–!@ë|þX`?ÉtAEo Í?á3Ï@ŠÎ-±ê?ò!#"'Ä?ËXòŠv'¿Ùµl]÷,¿äM: ºË¿ìZŸ2ਿíTi¿n¿ç˜Þˆ¶óUNASNone?"†¯5®¶ô?­ÏÛ"èï@?ƈ\m`µb?ÆòYÿ4Z?é¹³jú\ð?ÇUZ~o8 ?‹º+ØÁ¦?"±Eusœ'?Ô©‹§'qî?ɪoëÒ÷ß?å<Qëä?ÉFÜWŠ?«Í˜°L.'?"•ËTè¼Î?ӟ«Û7|ö?²eèýšxn?äsP‡_~¤?²3ŒÃׇ?>nô?À8?/Pœm(?҈sDP7?´Vò0`#?æ·ø›Uçì?´Y¶¿¿~±4FGL J1617.8-4418¿àûÌÉ¿¯@­ò>v]TÀ9é:G#«À;všÛ¸ù@9(_D´@=˜¿p?×è^"Ë?ïþ©SK¯@ÿSŸºE@£ñ~Ý֊?ÜÄF€íÑ)¿ÔùQ$µÁî¿êQˆÞ¶YC¿ïþð g?ï(J®kc¿ïý¬2ùQUNASNone?ØXUEï.ü?ȔΊÝã?ÜJ"¥`+f?Ì¢'¨/+?ƺL)aK9?Â`¶y:?Ï­½ÛÔ%&?ÊJ¾Uèâ'?Ìù$ƒò×?ÍÚ·™§ì?àÖJéú?Í°å½'¯?Ñâ˜ë¦ï
?®<2{?ÑÒ#¥>?·Êÿc€ü?ÜKCõ³Òê?´*Ÿ`Ÿ?҃uÕÌâ?»žÑŽ¹Ð?¼›yOå?Á!¿Y¬@è?ã*ÕñÅå?Æ‹AێÝ4FGL J1618.0-5119?çÞڇËf¿ä3™Š€!#À8aOZ±&~À:`ÇÀôQ@ ®¤¸Üó@¢ñÄÓÚ?Ä©ò­1&?¹UJ4VžÈ?ü­ÚB×@›cÇЎ£?êÐxR÷ô™?èD
úú?Èrè•U<H¿åe»¡k5¿éDù>oÒK¿ØøÒy´÷ÄUNASNone?…fÆ
WÅ?~Ëø¾D4?­­QàpG?³-4÷šzá?íϏÉϟ÷?³ã}@™?®ìÿÎÁ·R?±Ž#ëÈ¡?°íKb¤†œ?¹°îúùœË?ë󆖿S¸?¾´¯–—I?´IEº©'?—
Ðo=D?º1Ð4•ÃD?¤ZÂ֐-?ê0BRs?§\êËûm?§"ü®‰Ïû?•Æìn,'—?­Rer‹R/?¡Þ¸˜­Ål?챙Ýî­Ý?¦Åâ€=O4FGL J1618.3-4537¿ï«¨¥ƒ»@RÍÀÓgÀ9Úl <K
À:#ÍbôÁÞ@渭Ûð×@ݺZÚA@m">5ŵ?âm-êñÑ@»†Eÿ¾'@¾n¢Ÿþ?à‹)ßwtV?Ú÷;ÀöTÛ¿ê±­ÿ"Z¿ìaÄ@6Põ¿Ñ/AÁÁUö¿à3½Ò^FUNASNone?Œ›ÖÕ½Q?"îåÒßt?¦ R%×0?½yTofá?î-œnR»˜?¾8ÕÇ}=?ÚOE²Ã??ÒPù5ë?·éñËXr?ÅØӃ™À?ßîé=Úf¤?Ñéßõ?Ó|ÓPî£-?­ùdÑ£?Ähk¬ˆ?«u4Q"
Œ?á''<Œh?±ÌÏízÄò?×Ã@]ÇU?ÑDý£H^?=iùQJ?gä´²{ô?ä²¾®'-?ÑDž'©ç]4FGL J1619.3-5047?ï[±V7
¿Ø¸"*}ØÀ8¡.¢ªºÀ:¸ÒD@ƒ8XŒ@x@@aïß?Ë"">Ä6?Û²Çë¼|@®ˆã—?öþJ«ŸÖu?ÖîøüU¦{¿ålÿ!³®ï¿ÜkñUBQ´¿ç…`'¿í«a­šž¿ïrBþx%UNASNone2FGL J1619.7-5040c?u»†ú?rD+knæþ?¯!Î1ž£?°q Ça‰²?íâmµÛ?°×,ô‹ø?•]HW²?—TϬ¶}Æ?ÉIàvžEå?Â8‰´Ì?é´ø°ö?Á¿²][˜?¬©|pjÈ?ë "·úž?С–ŽË?±Qwš)R?åîœñíï?±P_ײ{L?Vۓé¤4z?EÓ¯-}1³?Ä 
?©&3Á"½M?êô´†¥â?©6ȟ§/c4FGL J1619.4-5106c?í:ôû•A¿ã°™?׆dÀ8=³/lÕÀ9×Ô)¸`.@!GÁntÒ»@'PǙ?Ñ
\^ûŽ?À½y]9!@^aµ&¾?ý|V[?ïÿúŒ"¸'¿ãP'7§¿ê"qh"¿ådÀÉß2¿åҗ¢¡§¿ç®ÿ\lUNASNone$?´âƒOÚs«?½âIè4?§¶Eæ´¨?²hÌ\b­?ëò"1¦F??'K6?"£=%¬Ï?žTÓòzû{?¸ýïd"¾?ÀZAGE"¹?ì;4Xê°?Àzj'¨Ìj?·|D©Ÿ¢??79[

?·è`_UP?£¿0Ðî?êk^áa«?¦BÁÂ*?lh'£â?Y.êŒØ?£Àö¼*ÍU?š›WÒ]?î§Ú, Á‡?š¹œÊùït4FGL J1619.5-5014c?ïn±Stœ4¿"ˆ&ÌêÌÀ8ȽÇvK·À9»òt&BŠ@ÚhŸ{°Ð@cnda©h?ʺðViÄ?И¹à6*@
Þ ²'/@%'~È2¿ïH¤´Îí?î<|½ÀÀO¿ØbO §)û¿ä†ÞvB||¿ê™XÌIð¿çï7@-ÌUNASNone3FGL J1619.0-5014c4?-\Æ(/?©Áµó…u?¬•÷'?´ éM~G{?íMEëèF?¹Æ¯ŠCµó?¨â
¯Ä?­i‰Ó1h§?º©C´¬?Àþ†klz$?ë:œ¶Ä8>?Â$ÁÐh¸?¹N¶7eQ?›l§IŸç¶?Ç¡9fA?ª4½øsd?ç%ʹÇ?¬p#{êsB?Ýˆ'e–ß?"oÿgha?–Ax^ƒ4 ?Š'eþ*?ƒ?îÇûй¤?",úWip|4FGL J1620.5-5729?¹\žÈÞNÀAÄÆnÀ9ßÊKM
À;‰%Þ¶Ú@
œß^@†{¯£Ç?ÈP‰°B}?Ægv[Ñâá?ÿòŸ	E# ?ÿUûƒ¯?ïˆ&_e@L¿Ô
£\ú¿æ†Ž¾`¿è"Ø¿Ÿ<Ç¿éâ<›<¿ïþØ
bUNASNone?ƚ^ôF?µÐÜ$þ‹?—5W'Ì@j?®Dë¸å›?韽½¬ì?·5É\Hq?Ðo>6ø?Àrì®w¡ž?™ý9p
U?œêEã—8•?æøW?¤?Áb‡þMr?הŒª¢(!?°[¤3Ƹ?³í³y@›?'¾j`?áÛô?ÃÛ?¯›º´r?Øm¨ý|–?¤Z¯–)?»©=ŽUðy?˜cʃh(¶?à'!y¶ƒ¦?¥ ¾|‡4FGL J1620.8-4958c?ëzî­¿Á?k'Úæ@À8s¼W3Ã|À9¤2ðîE@ÁÔKòç@Gòš¼¯H?Å2"{€ê?Ѫ¿±±=@€Âa8ÿü?ÿÕ©$|>¿î/§íå?ïoÑÿ¼Ž;¿â=à‹F¿ç˜§Å¬G¿ê–±‡Ìè¿èÈÔð‡½UNASNone0?k±ÿÀéÁÃ?pÁ<ÚN?£w€gìX?®†)ÚPª‰?î¬Ýø8—y?¯˜Y‹§?"*£‰¤?›âz?ÄmŒû"qK?Än€šg-?êCG¨"—°?ÄfýÞwÎÁ?ª¡øòÆzƒ?ˆOh	Äèƒ?Çdi!J*?§¹Dæ݈?èÇV‹EÍ?¨ÜΖ?p;@UÜ?ctš­?¨âÚËÍz»?š:ôðÕüÂ?îQ±Ü(§©?›U¯#3¶4FGL J1620.8-5035c?ïÒæ¾Eõ¿Ú¦lü,¶ÂÀ8A˜iòÀ9Ð1T5â:@!
"é3_Ô@¥ŒÄŸâ?É+å¶þ"?¾bcL€Œ,@Œ$›À»G@¨³Åê°c?嘱…K.?ÏÌ
…&¿æë%(®u¿æÆÕ½â¿æ5þßÄv<¿æU‡Ô>UNASNone4?—É÷¬'ä+?§C—ÿ?°ú¥È?`;?¶›ƒ½
Šj?í"[‰"|Ø?º©Ä§/?"APëÉUZ?šýT`âÀJ?ºÿÂI¿®1?À~Ú}ÌË?ëýý/i¿?À²·5¥—?²%šÔ'«%?"<LZk1?¹êZ—ïÇm?¤íc‰÷?ê~R}®?¦Ø&'bH?prc=d?iDÑ#B°?¨»
†Íû?˜‹Xx'â¡?î5nBaî?˜­¸˜(H4FGL J1620.9+4852?éòŽ¶š9@F>dÜY2À;'òvªHÀ<÷#ý5Je@4½ú¢É?ÿ‡ÝDUG?Ñ+ä<U?Ç#õ}›?ôý›yÙ
@·]`XZ_?ïÿþÞ÷¿í­x©_	{¿É£èg‡ù‰¿Þï0ês¿î
▸"?ØËWí»°UNASNone?íMöÁ-?±º‹ï•\?}Ýöº"Ý?~'Uö?±·°é{uF?°ðÿk­M?ü•÷þ?¡¹–*q?n¼Ø~Ö?wå74²¯?¤Wdi'®?ŸDºÏJmÈ?쬪dÕ)?œXQßÃ?"à)
ï×r?…¿zž¾Ï/?µ§j`Ú?˜´foÁ™þ?îšPäJûQ?‹ûʸË]?|fYÛ&?p	‰Ô{?¢Î°çM?‰ŒRÿâþn4FGL J1621.0-2625?ÖÞ]C/@0sï¿@PÀ9ÆÕ©²ìÀ;t	§H®Å@»¿Nßáý@÷d[ËÙ?̈́Q2øzÑ?Ø"@Îé@‹6¿y@*ö'©¿ïê~ŸBP?ïÁ0αÿ¿éåϽ—ûŠ¿ç¸ˆû¼¤¿ï»Þ§j¾¿ïÿö$´ë/UNASNone?äh"G¦èq?ÅH ÷Ù(?¨g«)ٓc?¦Éþ'Šá?Ô"Ævü²?Å%k¿Qá?êX9"'Õ?ÀW":¯Ñ?µ"¦Œ-?¸+é»-ré?·»?§Yã+?°µ7d?Ù8.<†ß?°™™8¡ú~?Ä)ðÀ«/u?£ïÐߌ†|?ÜãÏqmáf?¯‡¦ÿș?âÌÌ×y)?°¶¶zë^¶?»¡k@¾?¢Õ‡W8Í?Ó~=@Þ*?±œþ°^N4FGL J1621.4-4511¿å4kžxjd@
ª}>ïÿØÀ9ºÜ€žöÑÀ;n4Ïë@ï²>+3à@lX–š?Ô§]7¼?ÔïŠ|p>@O@4£v@+
y*¹<¿çtí²öaò?ïҀÖT5¿æÔÒ$ú¿â
Ÿû³j%¿ïÿyÈBúQ?î"ò¨ÿh+UNASNone?ЛõÖûÙÉ?¼DºCYæ{?ÁQ¦} s?¸^«M»8?ã]›u9öX?ÂÑÁ3÷á¬?ÑÚÅV«Ëœ?È­M§0?Ç1ÄaiéV?ÃÇ	'ʬá?áF,<OŸÜ?˽2ΠªC?ȃl'Ìb'?¤ç'Aê²ü?È»ÇH/?©ÚdNWø?ã°\íˆUP?¯8èåÙÍ?ÎÑË,ªÜË?°µÏ^#̤?°ê''? š;\¯?æ.Lb°gÝ?³…_'t94FGL J1621.9+6706?ßP×MÚ(€@C‡á2µ^òÀ;.÷<À<§]k"@;rW3C@§ÒŸt¤î?¿ìðXõ¿ºEik©q?ðÌgL?s³?÷,¨‡ª?ï͎É[ÿ¿êÙ"±ð*¿èÌÝÓ/g¿à‹ èBt¿ïüQ¿æ4}¿î¬é!í¸UNASNone?ïŸJŒ'?—%áËÞ·?{ÊØý‡M?'Â5-ù…?jÆH
|Æ?‰¶×¥'Ÿ?íFÀÖ
?²€-M¥W?•Ù•j6"?¥˜Ñ輄C?°T¬Ÿ?'?§©ñ&#?írƒÒr4<?—t=±ì?'6­æÝ	ì?…úX"¯â?°5ò·Ÿ?"'Bàrp?ëÐW'ñ?§-ê	ïÂö?µ'êê<"Q?¥1ãn…lé?¨®¸æxQ?'¨"ýϪ4FGL J1622.0-5157c?çáë¾nT¿øÓíçÐÀ9mbÙéìÀ:´&Nyá@䉱ïý@ã¬BÊ?ąÿb$?Á	WC¡ë?ýö5{âÏn?ùDÔ:ªJí¿åvw@(d"?ïâÜ~E«0¿å`i,"A¿åFÁ+Xô¿ìÞJZƒÚ¿½Ãø<èÎUNASNone ?´pTz??¦pÛ(]?·°V_õnN?µýòxúhA?ꈇ)r
D?º'6뼝5?µþ-½<š?±7R1xä?¼w¾×À ?»~îj;?é±Bm`k}?¿
å[?¿W×{{=?ž__ˆ'?¿¾!µ…?¢ðP¨Ø?è%0äï¨?§¢Ï$²<?¸ÃU¯0Rš?› h©ä´7?Ã_ø)ïÕ?¨ÃvSEv?è—?ž/7?¬Ôú"Àá+4FGL J1622.2-7202¿íÀ':+ŸìÀ/þKZÀ:}"ç¨ñ%À<|ɳ<ØÎ@¹âÖysß@$  0÷ð?ÂZŸÞ­?ÕðÖâz^@[è¡>©‰?ùzÛž?ïÿÝƒ(i¿ÝæüÅW8¿Ø¾\ý1§¿ä‡(mÀοì¾}ÖÅt¿ïÿ¤?åÉUNASNone?؛Ÿ«ûÓR?­"ü¤Ú?Õg­å/?Ã_MY&lË?ÒRø¦?À¶‹R3?Þlwʁ®å?̱#¾Eÿy?ÖP"…ë}?ËÖê«V¢r?Ç$p%ðË9?¿é#†K?Ñ]ÅxC?´ä•H_@?ßð"±'y?·ù/-tÓ?ÍdÍêt×?ªJ÷.†´?Ócœ"ðÆ#?§bQJ6?ր-<"?±iÂô†ˆz?Ö6UÒ¥P?«à'r
T¬4FGL J1622.5-4726¿ê'mí™K?ùý ½é¨À9V3é;˜À:²xþŸ3@®hÌr3ú@tÝdʄô?Èë¨Z&½?Ïl¡ÿCÂx@Ê:#}?ÿx-
TQf?î˜ÓÁ2º½¿à´Ҟå¿ç€ÔÜeÇ¿è¡Ý4ùÝ¿éTô¹zàq¿ï¾á77¥UNASNone	?«D&( ç3?¢'ôëu"Ð?²!(®·2+?­¼Àt'2‡?옇§H?´]nAô|?´Ì°z߃?³Ò°­ RÊ?»<
[èm/?¹'ó
È^I?éþý¾s–j?Á F]ËùC?Ã_et$¿á?¡ëé™)Ç?ÀIeúP'?ž º¾øg?çÍaø;ç?§¢j$ÿ·'? ÅbT̆Í?"h&TÒlÏ?µ¯¦GËð?•/2gy?ì=µ
Ê>?˜Ûd¨é4FGL J1622.7-4934c?àZk›"€?·†×J)CñÀ7Ò'D:ÂÀ9bÙéëÂ@J2Œðø@‹$ÜX[?Á5šìð?Ô¥lÞ@9É oâ?üç`¬"{¿áø"0¤º?î[R¡ƒâ¿àZþ¾·`T¿è+Öþ)E¿îW}à€ˆÑ¿ïýÜÚa
UNASNone0?v:™‡û
'?u8©œ,N?×÷+?dã?͏Ƃ7ï–?ã×õ-=˜\?Í®ßT?€þ°¥w?‡Ë¯d»?à‰ÆS'!?É؛Ëè÷Ì?Þdƒ ëX"?ɕfÖA?_?¡æ­·em?‹œ¯å`™Ö?ÙÐ sè3T?¸mE¹dÌ?áù"ôÀoÿ?·áú·<V?O4̺–üÙ??Ít0Pç?ÐõX‹"×Ý?µGê–5¥ï?ç}†‡îR?µN/ÖH±¦4FGL J1623.0-4624¿ïŠ˜çå¾@Fb\ìj!À9e3ÔBâÔÀ:àŒ]"Y@†zº±AV@ÛµûÏï—?Æë΅3±?®[!3‰ù?íºüÀ°^Ø?ù>&×/QQ?ïº8À»Çl¿ç*.<Sme¿êú©u°¿å>`"†É¿ç–&ÇUj¿à0«¼²UNASNone?½Hþ%n©;?±ÒséÇ?¦Ü	Mµ?†ØÉü'‡?ëàDË,öb?²øDµ°Õà?ÄdÅ^Ù|ñ?À:G{‡?°|øTKÑ?µËðo‰V?è×/À<é?ÃWä³¢é/?ÉÃÒ¾'ü?§'¢VOP?±rÞÓ?'…Úœ?ç`¯šÝ¥'?¨‡	Ûì™Ú?¬±*;?{͐A?¥zïm}? CÛ\&?ìæÓ
È6…?—›@Ò¾J}4FGL J1623.7-2315c¿»³ìT\@2"ëÄØíÀ9»øç
¶À;&ߢ'fŸ@_ºžLè@øb9°û¶?¯1†_Õþ¿XßÜÛO?´ýò^¬³¨?ÿG[iUŠ¿æˆ®Êä?ïüœh€òÚ¿ç%Ž?w4¿élëá:(¿è¢™ó[¬Ï¿Ú‰=UöØUNASNone8?ê¥Dà}U?½{,Jü`?'ïoï€?"ˆV°bsO?Ãþ€©1?¼-Î!<Ã?î#9~M
Ñ?§Ð4Ê•?"ŸZêz¢â?'ç–Õ,U5?¨¤'`z0?¢›±Réº?àhø˜DDã?±Ä˜7f=¶?²ºÑ
ìR¤?—vƏ
¤?ÚZ‹üa?°ó
3‡Qä?ãA"ÅÁ]?´.¤>aÐ?¢uÈýœ-G?&²M:{T?הĚÀ÷œ?´)ˆÖ¤å4FGL J1623.9-6936?åä/]ÜÀ+í²'¸#ÈÀ:]½‹ç)À<uƒ/ÊÈç@i"¨ò?ÿãf³"@?Âçښ?ܺ?×€
Qh@~3Auì@F-ðS:?íþ'›ýø?ä:ÿ°Nè¿Ý¡ªÌô»¿ßBL`€É>¿î9ÎWçG¢¿ïÿÚ«² ÒUNASNone?Ü>Ø5ãZ?ÄÄóš¢Óø?àý+$#?Åwšï4l?­Ýùkž£?¥)éC?èæN¨t0?ÆE¤$0G?ÀO'ò	?ÂY¯.k¨Ñ?¸ŽíB×\q?´zœ‰!Âi?Ô{[©‡_?¶s`F‹Y?áyљ.Ԍ?·Ò‡Žr0?Á"IŸ?¢TÀËÊ××?ç+÷Å,Ö^?®¢ø6t?ƓpŽn¸?¬tÉò?¹ya¡|ož?˜%&ñ™>4FGL J1624.1-4941c?Ü1	¾º¿Ã½?æõÂåÀ9eôݍqÀ:ß`ݐi@¯ÈV"Õ@Û`
†Ñ?Ò:Ùâ)U?ä_Ä@Œ70@[®¤Ã™G@!­Ý|é?åÁ¡ŸØx¿ê"ɞoc¿Çnיå¿ã؀_5ð}¿ëæÕÂ>ÔQ¿à¯ÖòÀ|\UNASNone2FGL J1624.0-4941c0?{w£qóØ?rðÉ|U€p?«5ŽmÕûï?©hªºûz¡?î·Ò>¸'?ª4¸Shÿ?¤êôyáï?£Mºúî]?«ÿa':žô?«"îyV?ì÷7¤·ó?°>èís7?¼%c""àl?˜{!
™j?È*Ø{DB?¨OÛl¬#?æuÈ×P'â?ª'SúÅ¥[?]±Ð'Ðs?"f[Ãã?µÛÔçüŸ? `ÖÌÔ¾õ?ìY—Ô{՚?¢ºA;w4FGL J1624.1-4417?ÐCžã@
—Ne¾¡À:8;fÀ;EÝhüBÜ@äÀ^g@ä…BÊë?˲&˜Æ
?Ø/s?è£B@WÝ¢&e?÷s7µxó1?ïþsè¿ãã'ö»3¿ÛØ´¢¨ñ¿å‡ÐO¹¿íهÆ2~Ø¿ïùñ]¥Í…UNASNone?¯C$µÕV?£$]܎÷?»ìUЖ"Û?´ìr/Á!?êŽBú›?¸S*—)Ì?º'
ÿƒÄ?¹ü҉8ÿ?ÍÕßmŠ½á?ǐóG@]W?åF×ã=`?ÆOUP?Ã~†|w? Ñ¸®	C?Ç>sq&ʁ?¥úmiÅÉ?åP܂/š?¬aÂ%ÑÁÌ?œÿwRF?€3@lñ©ó?͖ñc´ÈÙ?«
±0U™?ç²Gî8=¯?«':Á,ÿö4FGL J1624.9-4538¿â­8¡Î@®ò"z–À9½ï}Ѽ÷À;)²ì`@ub
fE@ܝ 6×?Ó¶@ï3?éDGÝå#@LRç-¡#@‹ä<€?ïñ©ûçl‹¿åø‰|ëä¿àø›ó-u¿îh—c^t*¿Þ}z¿ŽËµ¿ïÿí )k3UNASNone?Ў~w‡ø?ÃäFamvN?ÁVó«©>?º0¢†?ãcÙQ´u?Ƥƒ¿8(?ÄgÞE'ü?Æn¼44ôÎ?̐fÊD¬?ÉÒ_hoª?ãÂ#C|?ÌYl‰c¨§?ÊNsïπ?¦ûb¹èã¡?Ìöâ͑Ür?°ÄïòBÕ?â.ªPªeD?±/–©½K?¡¯L»þtq?ˆ½®Ý©?É,ÓH"à?µÖl¾Õ%?è™Öb7˜?µïíò@ÞD4FGL J1625.3-2338c¿®Ñ;\«"@1š'>[…bÀ9éÊ¥«ÔÀ;Î\ïÅ@
Ù æ@ê¬azŠ?×n†ÆX>…?ãb_p¨à@<÷S½@W?	*K-?ïÿwåëo¿å»Û¾,K
¿ç™ö!ãÕ¿ëõækÚC®¿ïÿÿÊPË?ïü!~|UNASNone1FGL J1623.5-2345c(?æþJ™¼µ×?ú
3qB?»ÔÀfz¼™?¹a~¨  ?ÆueÏÊU?¿`&	ÓÃ?àò"ד?ÑԜ\.+?Ôî1o†¤?ÑêÁÔm™?Åי
"i?À£Ìކq?ØeøÁ6ó"?°µ=æ(?ÇI!s"˜W?©4ˆ="!º?Ûõv…7ÀA?°O™?¹a™ZÊý\?¡0_Ã3?¾ÌbISR?©äü56ð?é3H]uê?¯ežÓGÄ4FGL J1626.0-4917c¿§Y¾{:翶aTâÀ8D*zýÍ À9Úqvdá+@<†¯Üüñ@)Á'°—?Ë;Á·šám?¢*	é¸ÀÑ?æÕÊ@qà@;†rJuD?áXsÉü7ô?¹¸"늿ê恗DU¿ç!Ú{9¿åŠ*@Ejm¿Üëû¼#‡DUNASNone3FGL J1626.2-4911<?xà7wÀ×E?sbÏâU™[?w$Ap;ñÏ?ˆvÏHÁM?ïŸ÷0n?‡(<ÜÆú–?¯©þ26B?«(P!p?"¤fç^{ž?›M¬Ùßé?íi(áè¾?¯<ý:2Ø?´/¿¶ßá?•f®j}Éú?³v÷
ˆuÝ?› B¹=?ë&XH?¡‡ÄÀPëB?§VûcÑL?•[ÇQ»ö?‡‹Þ–õ¨7?têiy_$?î(ÛíìJ?—Ç§Þ"²4FGL J1626.5-4406?äZWÇàª@£&Æ=f"À97RÁmóùÀ:þ›H"@Eªs]@yä"rÁ?ÄÚ^ZÔ6ù?ű9ÉOj@
f H	"@¦+Š¥?ïÁkoº£?îÆ>¾+Ê3¿ä¸R÷ô˜Ä¿âçfá¶hÝ¿ëw¡Aƒ­õ¿Ý+m×sï¼UNASNone3FGL J1626.3-4406?ßR©ÇûN?Å)š!Q>?¼ø~ÜËð¦?µÊÒLñ;*?Ùo6€Ñò‰?Å1¢Î¸ÈÜ?Üã8q'Ú?Ë ÈÎÿ‰Ñ?³§&ØÝê€?»^äê·?Þ3(W]…?Ê¿Ôeøù?àˆ3XNŽ?³:]8e&?±aù}?˜þ2Íɼ?ۂŒ¢?±üÉr)
ö?Ø)óÍ	V?¯®,¨ö8Þ?ÀZu´ˆ?¦Ô>
ø
?ßÎÞø©?°)7tV…4FGL J1626.5+6257?ïÿÇ»•²@Dß°Õ À;j‡È¶½—À=
eÀN@ uVÞ^¼?ýƒ_0Ð?É W£Õݘ?°Bq>±—?æ¨B©È¼@}¿AI¿ïÿÈl뻥?ïü¸¹"Š¿ÊÅ¡ŠSÖl¿å
"Þ|L­¿ÂW$T9¿ãkŸ‹K"UNASNone?ïáWwZþC?•(§¯ÓÄ[?'€âÛöm?&6rÑw)z?m0z"sþ—?•'êT€¥
?ﺍⲟ®?²åü¶D/?4™˜ïÏðÙ?F*÷¤µõæ?€·º‹Ù"ð?l¯¿ß¡?îYHUH?"FU²ÉF?x̬Ôw?x8š9b?«×±èà›?'&חɓt?ï̀bôÍð?dâ S#Sÿ?Cã='Fð?=mÿË·@Z?wCfÓPFÅ?deW[
Œ4FGL J1626.6-4251?ïþq[Êy@>­\ÄüõÀ9«ã°> ÍÀ;
»y¾1ÿ@ÊÅ&@ù5žG~D?ÍpÔ©e«?ӝÁÓÊm@íÛ¢R¦?ö­3²_
W?ïõ=߉'æ¿äS«Èp¿ææq¹€¿®¿æì´ÿP­—¿îí47³K¿ïÿ¤''UNASNone?Џ¬\$?Àc¯Õ]÷;?±0u6'ho?«.=ßßÀ?åÎ)ƒ
¬?Â7X}À?ÀEûIq?»à÷°›¿?Íä®Äœî?Å@K:X'?䨈<|?Ūi2Ôd?ÉøVÙJ~<?¥Oÿú‡`?ÅÀ î«<?§s~½ñ
?äÂ'o?®vS"é»?«$WäÃPp?âY
‰¡¿?É¥È"õ¾?«)øEYüÄ?çäHxö[v?®û['¡¼4FGL J1627.7-5749¿ÕbùõN÷ÀȞºjÊyÀ:%µQàÀ;ï 8"«Ì@|T{,q"@‡ŽºB†?Ų`$'ì.?Ûk_ý–™@èAYB@‰,™»þH?ïJ¶Ýw>ü¿Ò^©Ã(ß¿å"áu¿èì]60¿¿ïýؾ°»¿î·Œ~~
GUNASNone?¿tS¿Zš?¯)‡¨.ßï?ÞÀ_nF?Æ\@]'ï?Ù~ҋ¡ãJ?ð$É-Ã?Á±¿ì0±?ºÒ‰[¸2?Îüg*â"P?Æ}ý¡Îù?ãÔv:;2¬?ȓ.­3ù?ϕ68ám?«ùý(ú¼?؇¨ÝÖs?²pîÚ
Ž?×®O…¸Ö?¯^¦´+.?Ãͅ¶§?›VH©T-?Ý¿6#¨°Û?±‰íåҁ?ØZÄ?°³Dû¾:{4FGL J1628.0-4920¿Íè¤ÿ¿Öù¦¸&øÀ9¸<ãÀ;^ݚzj)@b6¬j—?ú{à€Þ·±?ÐÎҀÀÚ¦?ê £ylS@2µÖ\?þÃ]¸Aû¿ïþY#¯?î÷Pß@—Ë?ÒO¥¤ê°¿ä}z´ÒD¿ì"{ýýFg¿ïüÂÉ=ÌUNASNone?'T˜õZ.à?Ž"öžt#?£øxO(X?£((DTÀR?î5Ó³b¬"?§C¾G¾¡?«^—<0¿2?±Pý7ùÿË?È´ #ÿÊ?È?|7«?èîƒ=›?ÉU^ÅҞ?ÂüS|êí¦?¡˜.ßÎ?ÈåeÖ¡m?¨¼aD—i	?å'«;?¬ý]"Ÿw?»nãåOã¨?¦rÊ#ùí?Êfµ*ÚK?½S Æë$?åøv8Ÿ}ø?Â
ÎæPLh4FGL J1628.6-4553¿ÖG_}lj ?ÿ<û¹IbJÀ9DçW'Ž
À:ÔL÷)—©@L;´4ç@]X…Ó8?ÊðΉ»U+?Ë0¼
‡ÃX@2/ãšj@÷jt6?ïëÖï썿ä­úNw\¿åé¬Áêp¢¿åË»Š…) ¿îۚû™hò?¿›šOÌñáUNASNone3FGL J1628.4-4546?¥?m+Á˜ò?Ÿ'9N¬®Z?¢{œf¦çÝ?ŸB˜O³?Õ?í"OfÙwô?«iL#–.á?È¡ñjîQ?Ã8ªÊ:'»?µ]?PBÚ?µ€a?ç+ÛÒâ<?ÅÇW®g¿?ÆðSƒ9¯ò?¥©®¤Ä?½¾jâè÷<?žƒÅ½]Ï?æŒÂÔu?©‹{¨ÿç?´Šå¾3'X?—‰ªŸ©u?«£Q u?'wë™[¤¥?ë´q˜4‰?ŸJ¬XzÙ4FGL J1629.3-4822c¿ì*Ȳ®5?ÃÅR.¸ÐÀ8H00IsçÀ9¸ÒãgC@¼HOúê@zÓOž?ÉK⁔ë	?Û	읢'½@Dh¢€Èè@ÞN«´¤7¿Ì°¿%j?îÏ27Š°É¿æ€‡yÜdð¿ëõUҚl¿îpñÚ£O¿ë8¾"UNASNone8?|[n­+úþ?}ÿz7x›?²I;xé?¸Ý;oí?í~&û6Šé?¹¡ù+¸"?˜È5²ê?¡zø5ZW?ÌAjÖåÌ?ÃÎ"£Oð?è)cœã¶\?ÄeÞ[\+?°aÛÉht?'°Uör•?Å,ú)Ú·/?¥Á
'L?訅ü\C ?¨Î¼œ~´S?nœ~ªÃ?]$}ýšRb?™h-¤?©,~1rQ?ë;"\uìn?©tlI¨å4FGL J1630.1-1049?ÌÃäç1@8Ô³_=}9À:™Xù–YÀ<ÈÑÚRÇM@Í_íüG@ÖÝâžÆ)?̳üqU-?ïýò߆õ@ü¥zxl"?þƒÞ©Ä	/¿èQ)/»¯¿ãý›6QË¥?´Gz=ó>¿âWŸ¤¯¿ïÿÌhù¾¿Ú•©Àª€UNASNone3FGL J1630.2-1052?£=Íf—¨?¡eŸwr±?íêôAÀU+?«!+cq›^?œ%ÜúÆ
"?¤9¾"F?'pFHÈÃ? [âÊ؍u?»«œ7?©6ÖoÀ^?ž}bAÄfB?›EÃ&?¿ÌœÌ¤z ?¢|öVOQ?ç¾Z!í{?¬ š@f`e?Á I÷Ö´?¤×É¡5?'Ž0U²ñy?ƒº™)L‡?íãkAžç7?¡Sñ®S¦?©3»8Ä?PΘ
,4FGL J1630.1-3546?ê.¿Kz°@!Zt֐›À:o¶Ò"mÀ;Ҋ,l@ .á¿Î@´"¡ºÐK?Ñ¥_ .^?Ø`etÎß@ÿïÕ@Óo¦©?ïýœ
`{¿Þu]¿ä'"Ð=1¿æÐ6y8Ñ¿ïÿÿ)@k*?îÍ<(¥:¸UNASNone	?âþbf:?ÄnXð——ú?Â֕A)rô?»³Ìò˜'?Зñ^žÑh?ÁÞïÈaË?×2q…oÈ?ÌZ25½}?ÄËYÿñ1?ÃèbYÒ^?ޔ>áz—Ÿ?Ë|~í€è²?ÛV­r}^?¯¬dôõeO?ÈQ€Ê[?¥Ôü膐s?؀'¥
u?¬¯?€>7?×eDÜüðX?±N³Ð½p?Æ´÷üçÓ?®s‰þ‡ýµ?Ý@?$‹¾?²OùžïΟ4FGL J1631.7-4826c¿îçn¯hÁh¿ÇYϪ!Ò
À8ª/?ˆ¬À9ö¨y0m†@ )±`_¼(@$,!Æú%?ÒÂI;2[?ț:)Âq@Øm.׃à?ö­Œj1!?âÏàèãƒÈ¿áb×ÖK¿ç…¡êöÙ¿æ/¬*•ÕÀ¿ë¬] l‡¿Þ&«»Z3¨UNASNone3FGL J1632.4-4820$?‰÷X,q?"Cd{­¾¸?¨ßìÒbÙ?ªHlQªtE?îs¿5y!?¬¼<ïô´?"ñUo‹§?Ÿ}s‹Wª~?©âù2þ?±m¬ÜTÔÎ?íºEÁW#C?²õ-'Sö?¶7k{¿µy?—¹—Ø¡T"?Á—N	BÙ;?¥·ž2î?èÓ?7S?§ÿÜ*»²?eºVêrÄN?TŸ¼½`?›Ô ­µ¥´?Œ5?}ύ?藍§à?ŒL
w>߆4FGL J1631.7-2319c¿ïÆËŪˆ@0²Ž´cI{À9éŽuy)À;_ŸÐê@ͦ;2±@"î¿eÛý?ՔžÝü ?çSfåg1@
ÈÕ[ç‡c?ÿ"˜‹Q­G?ïõûg¿,¿á¿Ú@RÖg¿ë{τ7¿é¡P°¼¿äV 7˜s¿ïõr¾
—BUNASNone2FGL J1632.6-2328c ?ÝK3!tíþ?ÆwāÞÝ?Àþ¼—É~ÿ?¹Ê™KÃ?Ú5n'¦Rƒ?ÇFÛcË?ØŒ¨f­¬?ÐÅ©ù]ݒ?ۑê7LÆa?Ò/Å°?ȳ@™å?ÁwÇùdc8?Ûdó7Äo?°XÄ´kÁ?Ɖ¶«%š?«'liˌ?Ù¸¿ýò¨Æ?¯¨ž9Rþs?¸'ôӂ^ú?i¬Ê¶ÛÊ?Ð2Z›<?º?1Å 
?äÔ²8B1?º=×W|ë4FGL J1631.8+4144¿ïÿÿD¡Î$@EÛLÂPrÀ;zWûi˜JÀ<êîê3@!xáî'Ô?ûg?>Ú0c?Ð$a1s@?µO%,4fd?èË.Ò{bw@PHµP"R?ïö]¿Î¸¿éµyÿ ^°¿çëWÒNí?±·K†;B÷¿åreÊÞ¿¡°lnéÚUNASNone?î·âS0¹!?¹#ØùVet?:!òhuS?2¢Îώ09?¤M–è#ƒK?¹$,Ö5Ì?ï7}ä£u?–wwwÉõ>?T´—°px€?c'iËý'?—Ñ&Èd‰ú?•HdIW¥ê?í±‹÷/?"eŠÈ. ?qªEø'?o?åzêN?±\©ð/?""åDÓò?î1~m+f?•4Ñ(=a-?p†¸
y?fç›X­ö®?ª×H÷JGä?•&"¿¬?4FGL J1632.5+3839?Þ%¢ô}@Es£]gº#À;k¯{ƒ.À<™·•-#O@–A€h@EbÅÇõÍ?Õò£@ao?ã÷&<ª«:@jÉ¢uá.?ÿÇyü›F˜?ÞýÑÒ¿ê.!EÊål?»!Œ}ãkÜ¿á‰Õx¿ïÿøsCÄ{?ï¢,_Ú[+UNASNone3FGL J1632.8+3838?éÌâ|ÚæÏ?»]~ÍHºö?¹`'šXÝV?³$㥒¶?¸8Ä~Ïì;?²]ožj­F?ä
œj;â?Ë×$ØZ³"?̐FÏ/‹?ɹ¾Ÿ&]?ÃG‡'‡àê?µtAÛÑ×?æäBh%?¬·1õ+?½*%#ϧ©?¢¡FÁµCè?ÅØxeú‹œ?¤!›\ˆt?â gI8Fw?µIn"‰?Çî]h-X?³DÒß?6"?ϏÕ}¶¸Ë?¯¥ù–'Ép4FGL J1634.0-4742c¿ëlÂ8²Æ? ?áÜ\WÀ85O«8þNÀ9Õt1*Dw@y(

@Ývh<)|?Æ7d+xª?äÃf,Z@f×})÷J@Œ—Å¡_¿ì.
Ää ÿ¿ËD€7Ñ¿ÖÁ'¡…vL¿çëx‰~™c¿íÍsñidH¿ïÿXÛch…UNASNone2FGL J1634.4-4743c4?hà QòÓ?d{­.ê?ׂR˜¥6…?ËiõúŠ€G?ä&VӍÊ?ËpQqêà?…@O-<´
?;˜‹"_?Ò —("b?Ç©ÐÒ@¼?æZ³/'?LjR:̽v?¡—Íò?ˆbÔ_æâ?Ý`Ҏî?¶
õ-³~?àd–è2z?µ— ²Ê7?O²ý˜ƒm?A»›Ô?ÅñýN»?²%Zq¦ý?ê{"íœ5?²-§Tm}Í4FGL J1634.6-4324?éõ[¯±¼"@ýñ.ð®À9ã'Æf>À;,èI*}@ zËA1xž@ A`ó_ß?ÄkÝþ"…¿"«¦Â?ԕcߣi&@ØÐ,}·f?ïûvΓvj¿ÊQ§g'à¿ãÌxéö©¿âÊÆͯJÜ¿é(€‡yÜe?¾¤nò	UNASNone?Å°ÅñYÏÌ?¸¸Cé­ðr?" oN¨ÌN?—́VñÉ?éòË	4Eª?ºH‹o§å?Ý:s]*i/?È:êwaÝ?"¨£óø?Ï?'œÑ[Å?á#Ášêh?Çß"cÜ?Öß¦@P?°ðÜ3Qh÷?«_èÏÃW?+G'¾€?âÚ{ã»ß?°ç H.)?ÝÓ[´‰t?²
hL#6?ŒcBW¯Yá?{ALNôÈ?à¤ñÈÆýß?±âÚ$jL4FGL J1635.3-4159¿ÇÊç移é@
Ϙf"²ÐÀ9Ç DC%ïÀ:þìÁ^ځ@´°z[»¾@‰'¥R5?Õ˲[‹à?êùÄ¢0ìÝ@¸à†½õ?í(iå20?ïþ2Àœ'È¿ÚFUú³dò¿ì†úÆ[¯¿åÄd]øƒµ¿ïþÒn¥Ð?ŒÑt§FÖSUNASNone?×ÅŒ®dV?ÎVÐC	?Ä¥%!OÉÍ?ÅÎVz£–?Ýè[⩶Ä?ÏpÈ°*?·}µ+;"?À_I:öa¦?ުӇªã$?Ñö²p Y?Ûu¿4ŠMø?Ï»ÎW3?́
GRp?ªì53Š?ÊZŸj½<?­ŒÙmÐá±?â	ã>å?±ï‡XmñÆ?rñî]éN}?bzÔàæè?âöB|—tô?À|#ê?ÙdzMYpß?À]Éח4FGL J1635.3+4258?¸ ~—ãö…@E;Ÿ<pÊÀ;VzKöx˜À=WÃ5tV@©Iu¿Ê±?ý1ʘ?&†?Ñ:"Yd?Þ²¾äV×'@©äðl@
¨ˆ±>üÀ?ï 1-Ÿu|¿Ðl¸þæ¿Ô[ÉàhÚ¿ÞaŽºú½¿ïÿÒ³–šâ?ɀ:MèUNASNone3FGL J1635.3+4257?ï<å ¨lM?•â,ÀÂX?‰ðô-¦ð?ŒÞú^wo?†Õ£Ï·Eì?‡4<àGZM?î#Aq•°?«ÿQ8(Š?"zzÞÅF?šxØ0Ø¢	?¨­DÇíM?¥"G3ÐUp?êš–ñɂ?¨(&ª'-¨?¶4C‰á	?¡Æk—Q?¸ï#çÒç?›×ìNHZî?î¢õR(Íù?Š"µ·?>½›ý3¦?}:¹Hâ?›b˜é
7?''éP–‰4FGL J1635.4-3249¿æ"zB]¿ñ@#±vû	 À9ç$Ã-èÀ;²F;…è@+hÌÅ@è¡ß¹8›?²¸yƒ¤?Îɹ‡uª§@§æ;2Ûõ@ür׸ä?ïÿÆ>"8¬?±é""xi¿åHpSO2¿æބ 
Q!¿éMd6á=¿ïüNÀ,€gUNASNone?Ó&öž«ú?êÂ=
I}?ÄX}Òq?»éÈ:ÏÙ«?áV'Õ¼&æ?Ç*/¹ºMÃ?؞ø±Ãä5?É«õš½¼c?рiªŒ¯B?Å}ÆøÎë@?Õà£¯l‡?ÇêP~³hò?Ýo¦ÌÀÁ?¯Ù¼ÄdD,?Ãe$®§?¥dP'¿?"?ØÝÕíaçí?ª‡TLA‰Š?ҡœöێ?£kօž?ÐéÑ«J?ªûŸt?Üu('^)?§ÖçÆ$Ì4FGL J1636.9-4710c¿ÓTÁðyÙ? š&	ÔëÀ7˜ÜïY¿À9IeVÏ@6ë¤~O@‹jËG?ÀƇ8n—?ϵãfÂ+ß@qIáËa"@áIÈ î?Ñ~Ç[HÐÿ¿ÙÏUàW¿ßgçšÙ_­¿éb—oîM¿îàWÄ4?§i™v´UNASNone3FGL J1636.2-4709c4?sÀ^bGÐ9?seBHCèX?ÁÎqL_?ÁÏ<%­Ÿ?ëdþfèkÈ?ÁüHÌ
s…?ŒÕ?Ë4
ð?"*üÉoé?ÄLãß>Ï?¿È"ã݀q?êyr	|?Àï‹Í$?¦(]szø?‹þ®½mƅ?ÐÀœBK—Õ?¯÷HKíL?æ=,¨|f?°;]AêQ¸?K_ %Ð?>¿5¼¤[ ?°wKÕ@o?š@÷@Et?íêQŝQé?š\
EÝ4FGL J1637.3-6325?¸ÎöîØgÀ%«ËÉdcÀ:¦°ÞY½À<!<(F@ý'_d@@@¡°¿P?ÒJ¢e›?Òò=ºË˜@ëó{??û0¬%~é¿ìîX}šŠ…?ï°*À¿ãOøØ¿â†ðY|s¿ïÿ']<9¿ïÀöÕ´ÒÛUNASNone?â<P2·tR?ÅڎȖ??"'D-("?$ÑØ?ÚO;W¾•d?ų͉çBU?æÐ-;ئ?ɝ=&ë‡?£â颜
Ã?ª$?qŽ?ÏƐ§ø¹ú?ÈQ á+4?äÇâ~ÐÍ ?®ÓžôQ‹?º°£!x?[eí
V&?ψ$¬
9?¨äzÏÞ{?æâE‰\??©Eɜá?´ÊéC¨'3?žýÊü3††?Êu:"Mé?¦IåkG4FGL J1637.5+3005?ï%¥šÈˆ@Dd| À:ãi:V=#À<‡CrE˜@ùrŸ.ÙÝ@~³¾"æ?ÆÕKÚt?ˆ ×üUÑn?¿Øš Õ£
@ÈYÖ5+[?ïü—`uÖ¿èNƱ¿åo—Òïü}¿è‰/žÔ¿ïö(°ù1°¿ßÚ{v˜ã'UNASNone?ï¯CªB£3?«à̞Y:P?€ûMËÓ&?«å"*†:?`xh†-€¸?cÌ/æ}Á?î¢9á!?¡ÆV·¯c)?qü(œŠo?{CrÎ$?£œê®]? 9éGcÝã?í"NOEü?"ʁ¯Ÿ?Œm<a!?}œu®Í&.?¯¤c×<‡ù?¶òà!?·Z)?ŠÊÖµ0.?"ˆ¾JÅó?ƒ˜7í%·?—"°þOð?~æÿFW¿4FGL J1638.1-4641c?Æò}ûZC?Ê¢œâú5¼À9·ÛàfÅÀ;`®­ýÔ­@ §è½@G'Ñ(| ?Ö©Q2!»<?ïÕÿ™'Ú@ò¶ä-;¢@&½cÎ0¥¿ïõ~̹­?ì!S6Þ¹^¿wõÚã¿äúf¼Í{¿êï…>BÛÈ¿ïÿåþÌúUNASNone8?›ðŽR
zq?"pžâ?ÀU)µàQ?»B'ëúQ¼?ë8Ã?¼Ð'+™Û?žaߗ®Z?¥9ÀÈBöb?Ùmb)··?Ï
Kâè²?âVF{æ²?Îý•ñƒéÞ?Èp'ü"—ç?©gF¥Â›2?È 	Ñró?¨™ÊæT?ãÛÙ'F?¯bÑù4g§?¯ù÷Øàú_?šNÉÜó?àbuå?¾_ñI…a?Û;ÖùÉÖé?¼Ø"I¿*i4FGL J1639.0-2727?çÍgÚãC@)"¨ŸÆÚEÀ9ÜZ°O¾"À;¹¶à…@Y¤¼e@컚ua¬?ÃWq–ë?Áûÿ)ì7¡?üÖ$ê›í?ý['l×CÉ?ÏòpËD7¿â:7žÒ¾~¿æµŒt)¿á›>¤€¿ë¬`Eºõ¿ïÿÿ>¹úUNASNone?äç;à(	î?Á¥_Aœâ?¬Þ:™›?¥Fpä	=?ҕÈ\»ñ?ÁyìÑü"y?çqÑí߀?Äâ#\ü‹Q?± #¼UÛ±?±ìòAi?Éh©æ"&?ÂW¨`·?åQåì·7¬?®Ð›9Øa˜?³Ý˜É`?œ7©nö	I?ÐdÌÀ_K?ªÇ蹟[Š?âfn°lNª?§pÝ!Ù|Ê?ºT†»æJf?˜B¿ÐDË ?Ԟð-Ð?§r…÷½õ4FGL J1639.2-5638¿èrÜ×˝À+äøé‹À9ñ¿ä†ý¶À;¥0°¡óÛ@sYùñs@ÝڋÒ0º?Ê÷8[;:?áÉø;æ`@:k
•ù@n‡/×?ïޝåX´Í¿ÝYßð@¿éÕá"oA¿ïýð@o\¿æ)f–7Š¿ê°ßьO.UNASNone?á°x™Mr?ǥր5?ÁIµ"§êS?¹ò«!¥È£?ÓúòDùoô?Ä%[z8Þ?Ç(ab•}?ÃøaìO	?Ére&Ëj?ÇZbµIçã?ãÙF㝧Æ?Ê@y@=?Ö#Llõ?­x;e?̀Ì3Ï?¬nn9Iûd?Û¼àvªy#?¯"½$KHV?»´ò¹áN)?›ÜãÚÏÅ?ØDž]æi…?¸Ìé"ÀV!?à%žùСx?¶#`b7#'4FGL J1639.2-0946?à¡% ˜H@7¡Â # –À:òþUÀ<åê«%@ òæ0v@°nºÈ¾J?ăùdo¿¦|c /Ø,?åKÕ@Ž»o?ߕ<¯« L¿ïí	î–K0?ïP3ôú€¿·Ux­eÔE¿ë¨F`®_¿án•Š¯œ?ÔÉÞZ鰈UNASNone?µj?¦_ö·%/ã?c7'X"¡?jøi>»Ð?¢ô‰@?¥—ź)"›?鹆2g?ÆÔzC&[?°Œ»¼Wc‹?»¬Ï¯—ö?ÀӉÍœ?Àܾ'þÂø?ëÂ÷e™Ú™?¡@<_?†ö?—8­ø›Öš?s¯õ¥?¼U
5"?ža3¾6?ØZ'~2R°?µfÐAG"Ú?´Km­Q7?­»XQZ?áII<¯È?¸R¦ÀúÙ4FGL J1639.3-5146?Ô¤FóÑÀÊÀ
©9û¤QÀ8Z"ÀÀ;0r›þΨ@J(KK?ÿ'%hoU?´Á6þCè?ÓÁêAÞG@ Ã{®Í…@­±~'­¿³1¦–,QÿÞAMÝÙd‹¿Ö]B%iq¿á罞±†u¿ê0[²®=–¿éI˜ÐEþUNASNone3FGL J1639.4-5146?ŠciNžÊü?€Û'#Ý?éó^$Tµ]?¼)]Î5µQ?ƌPÙÃ=Ý?»y²Þ '?˜3x%?›»†[I?ä%^Òºœ?É,cvl_?ÖdƒŠØÁÖ?ÈÝ0‹>?³ù"©;J? hУÂò?夁‡k(?³§Gl™ß?Ïq/}µ»?°L'à´Nß?¡Q-OG?ƒ¿Àâò+ÿ?ØïX¡<?±WHÜ«?âçu~¾M‹?±¼8³Úõù4FGL J1639.8-4642c?Ö<ë\ž«@¿˜ÉF"'ìÀ7Ÿb¶®}À9,5Ý1žÞ@ }Ö§œ@¸TÛ#§¥?¿÷w›BF?ÂVŠüñ}@";~[O²?÷õY"š&1?½ï¯aOÊ?îØTTëꟿçue!ÂÈg¿æ/$°¹pÏ¿ë]"3¿áHΙ«UNASNone0?xD³­˜=É?uêÉñ{@@?µ'mí}â]?¸Ö7u?íHÚõ8?¹[2Xw3Z?"m$Dæç?"Pó"ä?Ð>ð¬ñ£y?ÈÅNú)?çŽÓB¨?ÈIÁj®?±spìëË?'ør/îd²?È@âYÑÍ?±HÃSn6Ý?çÁ'©åî?±yý?ë>i?MqÁgÔ !?A¹ûŸ•]$?¶[í¼E¬Ò?¢X¦ðèë®?í-%ØU=?¢t5+ÿpõ4FGL J1640.3-4917¿ïó‡^ƒ˜ü¿üºüUP"mÀ9(اÌbDÀ:½ž¥rð@úü¹úb1@B_@Ø?À½ÃÚය?Èú(Óo@	¬Ÿ›;ZI@,òý8%?ê6'¾5Û.¿çj®YÒY¿äH$[ÿÛ¿ä«@ "€¿é ¨¡Ê?ª¿ïÿª¥Z—üUNASNone3FGL J1640.6-4917?ÀÃVôI?²[Ax"Ã?Å°'|]Áª?¸öBU®5?æŽEK+}T?À"
š8,?¿£ª¢§B?·TÍò†_?˜ü¾¥"%?¡
̲ZÌé?ëÂŵã¶?¹:eKDæ?ÑÓV"-?®ÒÞ@N?ÀLÿõ? Hzî"©I?ãmP5ì?®m•6ñK~?°¢:˜×&5?—Ô'ß°?¥kåφ±¶?düQ¢í?ì"úOì°? †‰)vý|4FGL J1640.9-5853¿åžÌ"GÀ a«°'ÞÀ:*‰*¶ŒïÀ;Å0[žŽ@Õñµd{@Èb?ÍJ|Pª?×	üʃÒ@‡$Y{œY?ÿv"¹ªÎ?珻"–$š¿Ó¯¿uÌ4÷¿ä•"¦óõ0¿ìL<"Í¿áN3i¹Ø¿ïáü^à¶UNASNone?°ÄI¼®q?¦q§àæc?'¤ªäªÇ?¹wðb?íRQqXsù?ª[ƪ³£ë?ÔAYÂr²ô?È)"Nn†€?§×ÅC‰ß?ª<2™Ì»$?äaÖÆÒmè?Èû|·âÓY?ÙÞ»&HV?®"»¼ÈÝý?Á£¹Ȫ?ŸPÁÆõò?ݝr¢MST?­Á( 9?זG(²?¨Ãäl‡¼?´ô|LÛ,J?ž«îºü|8?á–LâWž?ªxJŒ€q4FGL J1641.3-2908?ïÒ2x‰e@&—PÁ¹sTÀ9}'šy"jÀ;š™sÚ@¶Ó'7@ýÉÄڐ?¿ª:P³Ì¡?Ö¹;àÖÄó@'Q~wÕ$?øpkܜù?ší"á4¿à£À9 ¿è:T¤MR¿ë³݆Xt¿ïÿpž"ÀI¿ïóÛ._"UNASNone?Ø!à…RÛ½?á:¿ºS?Ô?kœh‡?ĨÛŠ#X?Ӟ³Þœ»¾?Ãl–°˜i?µKDIð7?¹9‰Æ¢FX?èx^µüö?ÅÆ1>$,?Ãyýã?¿îYíŸ!~?Ò¶jž‹??­mííoT?ÕHIAíf?°¸(£!±?Ø¢‡X?°'D"mãC?µã7ï‰ú?"pˆi ?â£nDÚ÷?´é9N¡á_?Öyë'"?³eIXñá…4FGL J1641.5+2017?âü8­›"*@Bª\=îxÀ;ÃcTc.¤À<ÇÉ"a:@#gß?ùiþ†ƒ<`?Ë*'Wގ¿£à­Õ:Úq?ÚÃE¤ú˹?ü¡ô;ђY¿×Ɉ'N?è{½`H?4¿Ùu
ƒ'šr¿ÚÅéï'î¿Ùn¾ú|2¿Ç]ŠÊžÊ0UNASNone?ïZ%Žä5?ø1&x?Q.2gÿñ)?ODu2]??"¨{g£z??S@îÄ?V0z1?¬ÿ½É"?m†ÜրX!?|ª"âZ?¦LϐWi?ªá˜@++Š?íÜ«ë™0ð?"'^+f¯?t6Eìîì?dÊ =ÃB?¯®xˆë+?"²à,Ïùm?è~öQä˜3?¶VÐ Öæ?KÉÿ?Šü"vz'?Ìt»Ý/??·:ÞQtÄ\4FGL J1642.1-5128¿Å^23ó'LÀ¨…·d†À9¼i"ïÀ:Ý(8-n@"v4åç@_­)™V~?ÒÊ"Ýtæ?àƂ@³½@e¼¦äÜ?ôÇ]_Áq¿ÕþŸb†\ü?íìk΅3±¿èIˆÇì=¿íX›7(‹:¿íÅý¥²­¿ïŠÐsJzxUNASNone?Á1Ú¤ºû?·("·ŠŠH?À™ªÀ/2?½WÆõ½ß0?çÈQ…u?ÃÃ`½)¬d?µƒ¾éì?·ˆBþ6å?Ƒ×öœ.ü?ÅÎ3Ñ?g¿?ç·¹¡a?Åáö"̜?ÃRUû¢Ã?¢zåC©°?Å[" yÓy?¤å¦-?<Ì?åԅÑ"¢q?¬"ÚçÁ?Œ>̎[ž5?rúeš½©?Ø`©\¿"?´m9ª*?ã^ôù1Å?´=mÊ*_4FGL J1643.1+1436?åâŽm@ .@AuY_í¦aÀ:ÇÌW\À<8Íl.ýD@ßÿ|Øï@;ßY—K?ъ<6\?Êæc¡ºû>?õ¶¥ÉRÄÉ?ðûpú,?ïdH•:¿ç~(kBn¿ç$›?áíE¿æ "@º¿ïÿk*M±?ïú}¹©"UNASNone?îzˆè©å?§¬ù8îÅ?'.ïr*ý?¢\£Ãˆtº?ž€vx˜u?š*‡Ùªd?é2To?ÄL‰º"Ö?·'	0žß?¿h5ÏT	Ö?¼ÙÞ,.ͱ?³ÈC‡iw¤?êÖ1$?£ÇØR)•5?ªr©A,‹€?™}¢iŽûv?¼"?8Áú?šòÇEê?æ«í8_,Í?²Ô¢""S?´Í4÷U'?¢Ÿì×ÁŒô?ÊéÄ¢9?¯«ÐîÆJ4FGL J1643.3-3148¿Ü­³…g!@"|/øìÀ:‹O—ZÀ<DÂ<Pg@9!­NØ*?ÿ?èh3Æ?ʓù\!éà?ۅÎÁC¬¨@‰È]ÒC.@÷é¶9¸?ïôŽýß>i¿çö#]R@•¿ÄQj‹¿ÝӇ;žÍ¿íƒ9¿ïýPÃfò}UNASNone?Ð?Nʽ¨e?»'ׁøš"?ÆkÁçÖ^?»ü+9Æ»-?âEh «£ö?ÂRB¼Ò¬s?ÙKÏ~•ƒÁ?ʍʀ íî?ºPÐMõ?¶'"üÓOÉ?àþ=kša?ɪì%f?áìKÐh.7?±Þ:Y(?ÇùŠŠ;"¸?ª¤Ë§Ædl?Ð*£Ùµ?§hå~ñ›W?áð¡?¨
trJz??¾áùç¯éã?¡"ò­¶Þò?Ö¡múÂg?§\²l¿Ëf4FGL J1644.1-3055?ԛN·ü@#d:æ…ÛÀ:&k/#:À;žM³9ä@ÙDÿŽk@í£3vO?Î,êâúâ?ÔÉÍéØ?ó›ªà?ÿ)µ@>3—¿ï8‰ÿr¼`?ïò)}§ËŒ¿ìJG¡Õ'd¿Ý‰LûoV¿ë³_¾V'^¿ïùVbã$'UNASNone?Ú_ñPvü?ÆîÍÖˆi?©G:|À??©îïµLVZ?á;"¯øùO?È6ÅýQè?ìŽl†'Õ¬?ºWàè`'•?'õ\þ**¬? ÿ-6&¡E?¶ÏD‹æÇô?¶Û1õ"?ߥŠ'ÞŒ?°&‹Ý——?¶',_©)ß?›VM½Œc¥?ÚЪV7)m?®F¦""?é/<P¢?ª¼iíXX?¨t6Å[^P?"¨HCS	Í?Å&¥]f±ä?©-¨z€B£4FGL J1644.1-5009¿ïlÅgJ3Àž"B€À9†³k¢À:ïü£T-@££Ùäbk@1n¢u
n?ÓQ§àY?ÛÐo¼@I[»èxû@SóÈF*?³?¼X‹\j?¶8ÐÁy§¿ãRAK#êÁ¿êÞÊl <¿ïñà¸<?ízVs'UNASNone3FGL J1643.6-5002?ÔއùÖñà?Ã>æ•a©?¥›.ãÁq?£}åŠrÒ?ä7	!Jù?Ä Áòyf6?Ë6õ;&?Ä:sÒÜ"¤?¥<Àh'?ªÇ/Ñ£u?çÞ°ÁZ­h?ÅJAU9@?ÍP/gcç?ªiBÕ¬Tó?ÂbþrJT?¡,Z'NžÀ?ä<W"'â?­G4+¶?ÄßvÐQ'2?§ƀ¶?°üõÑü?™b3uew?èÄ>LLûô?¬W«ÖÊe4FGL J1644.8+1850?ìà2u¦¨Ô@B
Š†×6À:¾B°Ž©À<{ˆÀ-'@Eïµ+?ý¤òÈßØB?Í[JiÑK?ÐÈ b‹l@ö¹!õN@ÊCt
¿ïÛ^g"d?饣'·Ôî¿Ñù1Øýˆ¿Îa
6u¿ênÂÀÚPC¿â—À±5—'UNASNone?î7:w߄?¡	Ŝb#à?‰ý}ò`àã?æ3aÀF?¦
;éυ?¯o-N?îú°™ÀDˆ?›V4M"0?uHÆÓAÃà?º°Me?›W»&þ?•¨GV›bà?ë›=i­[ü?£ødnùÞË?¤…™os?'Ão"ýb?¸ã‰åÝf"?œÅ¿×B¾p?íDÚßÁœ?"'³²€Î ?œ££Ü!ó?….´²eˆ?­¦€2ÕF?]Ž`ä4FGL J1644.9-4921¿ì/ñÎþšÀL,äd™À9@4ŠKGýÀ:°Ñ®³Ý@é.¦†'@
–»˜Çã?՘L};?ç}®ˆ@•ƒgþí?ú™¨	ôËn¿ïò°Vt€Û?ïýí@
¿ê\ܤZé¿ïÿøsCÄ{?ïÿKÚÉ咿ïÿþÐñUNASNone?èúÖ$áÜ?ËC$¬á?·ûåÎÿ?Çš›G=?À´ß=?ÁàäO)¹¶?ÁbN¼ðøc?ÅXÁ+«‡?ÀÏ#c'9?Æì÷²Ù?çs£w߀Y?̟6tBì?Ê\«\³¨ç?§dâR»Öi?Ê×Æyáï?®S螓K?â²ãŠZÏ
?°Z€rL7?±Ï'\´%?±<c1 ì?ÑÉÙS²¹æ?ÐH`"W?äéeÛ‰?ϱÞ~E;44FGL J1645.0+1654¿ìvëÞy·@A­¸<òϖÀ;ÇvK¶¸À<s;ʱiš@á4"å@šoŊ¹,?ÏD¤_E_Ü?©ì^¤Ö?܄YÒÚ-?ÿN‹‰
«¿ÔʏZÑ\Ô¿é^`¨·CÏ¿áØa@Þ°¿â!†BNÚ¿âçÉ0`¿é$UIÞpcUNASNone?ìÞM '@¡?«7YsQ?oìóď?bOþþ?Ù>?¸¢†\Ó?ª¢žéYÌ?pxÿ?œèDu€?h˜¹>†ÞR?r-0ØýÀ?¢›Íc@/?™Ð({üÁ*?í"Ö-¦?•Á†[6!?pýáž?q3Öóå4Ü?±+.ï3hc?"¢:•Û'?ìÀÇ-£¼?•;V>R{?vfV½Ç?d7œåàŒ?¸ž«a'ª?"×xŸ<yÃ4FGL J1645.1-4123c¿îÃò)
ü~@ý+9i®À9ËQ•	ÖÀ;R"nmØ@ â"ÊZW@œ	€²B?Ȕ¤ý¥Ý ?ÏB¨Ã
†@‡p_
¬'?þà-,3Ë?ìÖ`^åh¥?ïâžá78¿Ü=oa·ªý¿Þ3.€›ñ¹¿êãs¢¡¿âüýKð™[UNASNone$?¬XƖ?¡1Êeö&q?³üÓý0Ñh?¯"‡w5?ë¿åZÙÙi?³t±dz¯=?ÁÓlÖOû?»þSëd{(?ÈÕtôQƚ?ô§NÛÀl?åUǼµúZ?ÆódjH_6?Î*ùŒ©:H?¨ÿZÏü?Á¶+e6þ?£p"Ñ|ð?ä»Qüc®?«LÎt5@§?Á_š£[Ո?¡LÙITµ?Æô˗æ"?«–ÂnÅZ?åêæq/eÚ?°MMôÁ/4FGL J1645.2-5218?ÁƒßnÌ!½Às©óƒð»À9¼)DœèÀ;/Ââæ@»ÑOéL_@&t	?á » Ôv?Õ¡}]ù°[@(a´Oþ@ÍüLÂ%?ïüÒf(S¿é1ÁXÐQ¿ë¯¾¿Böu¿ãr®]Ëã¿ïòÔÔK4¿àME}¸'ƒUNASNone?ã3["~Òq?ȉ!üqÁ?ˤéä‡Ó?È.
bÙ;?Ǎ¨	ê.h?¿¼1r1ž?ÈÕÛwO%ý?ÂÖçÔâï?°î¾Ô¯HQ?³Ÿ†®1F?笱G–Mw?轀¿µ?Ò)€¼Â–?®#/ð|V?ÅŠí<-?¦BÃå«OŽ?ᩜæ[.ª?°5Èzï	g?ƕIó[¢Á?©[mãçÕ?¸®Õk\™?²Ê£ÐUc¿?çDÒÕ½"!?µü"fB¹Ü4FGL J1645.4-5514?æ2&
À*è},{‰À:¨`ÔV.À;ÇÌÒ¬	ß@HýwÞ@DÄ¥¶ÞN?Ԃ¡z¹"œ?âövÛ)@©G{¿"@Õ†å"?ïç''kþ¿ãPR]šåÊ¿æk_)[C¿ë˘_1鲿ïÿÿ" 5•?ï÷üß¶´UNASNone?ä9Ad%È?Äxg÷}‰?¶Ë,μOº?µ˜w,‡Ù.?ÑÚ²\
?ÂVˆ•y('?Òná†ú@?ȓ½
µâû?´˜w}¨á?ºõÝèé#??äF-"*ã?É^?½eBC?ÞÁzΧ?°æ·¨ßËM?Ő̒
C…?¨8s/[X
?Övˆ²~–?­ƒï,?Ò*€5¤Ñ?°ú"3…)?ÀMýÓÐ â?ªÄ9"?â×1Êñ%_?³À…àPC4FGL J1646.5-4406?¨3(<ÞMk?éÀ̾µÀ8â­Yiþ¡À:PÑCT§@#úäY€@²¤}"jŽ?ȸ=³™?Ã5֟™?ü¸n;Fýë@ã[:¹9r?ïþôÒ¥Sâ¿å—ñŽM5=¿à',)S¶`¿æj*sq¿èï€@'&5¿ï딾h…ûUNASNone?–Øl/*/\?•ê Ö²ù?‡±É)? ¯©ôyN¸?îÄÿ=îT?¥íÁâÒ)X?¨ðêR&R5?§³K
ËØÉ?›ôrF? Åm~žô)?í˜yºÿJ?¯W‹a"ô?ÀÇF,Vل?£6]1_ü?·_R¦Ä?ÃD)o¤°?èí"Š•q?§~²µ¡¶¨?ŸÄho¯s?‰'Ù³
ˆ?™³ Ä~Ñw?ïŽq³U?î4C¶^Ø?'íB²M¡Š4FGL J1646.7-2154?ïýòñÆùœ@-ÑÌÙb…À:°«."À;a_–i@6ãtt@Z¹ÚÁ6?ÈjkØLˆ?ßGX"%"@3̼ܔÁ@ ŽÂ%?ïÿ¶~¬®I¿á£qõáõ¿ãY.¥.ù¿ê!ÎAÒ¿êՀ?€sƒ¿ïþP½Ý›§UNASNone?ÎFëÊå^?ÂU6óRø?×'…2oÈ
?Éí°HÆ?ÙµkWªÅE?΋«ôÁ?Ð{il Å?͎]r˜ÉU?ànhUùLì?Ñ¡cß×?ÍOŒ…AŠË?ÅÌㆭ I?ÊñyŠÕõX?ªç«d1…?ÓÖúé~c'?±¢N™?Þ°HQ¡Á?°Ä·ÝM³?ªèà=[/r?s|°&n?ÞÕ¡¦&õ†?¸¨%Pi?ÝÍBR-¤‹?·J=#¡4FGL J1647.5-5724¿äñ`̸CÃÀ˜Á@§üÀ:
·­€×+À;­ŽŸj"ó@¡Öiƒ§?@*~áS?Èz€ú'V?À¾ß8à^?õu°Ðî?ô¹#ØL\Ð?ïûÅs<7¿¿âc'·Ôî¿çº‹·XÇA¿ìõËß	¿¹HÄiüÉ¿ïú¤£|UNASNone?àÅòêN˜?ǶB£`—?•G)É΢?žÙEX²õ?Ý#WeŽÅå?ǸpÇ?ÔècVHJy?ɒ÷5#¿¿?"F¸Oÿ?ž3ÃLçˆÍ?äñ™çD?ÉÒüº"Å?á¦ÊV–°d?°V£+°˜?­\ììJ÷q?"†]™š?Ù͵I@H?®íãáúÛ?ÜBÔ8NÔ?³ûq,{<t?©Pñdä-? Hƒú&
«?àI†ÍŠ»E?´‹ÖÝÊP½4FGL J1648.1-1547¿îy¹N'x@2Y"9ÞHÀ:'÷†®À< aïß Œ@"tX€Ÿ¢?ûíÄÉÉN?ÄQÚþ"ÄC?¢ÎéõÒ?á#œ½:ˆ'@J†áÛþ¿åµv9B@í?ïý
q؊p?Ô÷dÛ¡Ò¿àä#á0±ú¿ÑWÊ¡ú;E¿Õšü›¤ÌUNASNone?y_­s? bÞÑ
?f©Ö¶Ün´?dY¼P~?¤Mþ—aú? #œÿ†Ÿ¼?îûÍFås?¤7ÜG'"l?[‡2å[‡)?oÊüK6Š?žÍãôûçb?£Ï^êOüj?ì,»éú—ƒ? ¢Í–™‹n?"Z)@@â?vMÚÖÐ7?¼ۈ#'œ?Ÿ9–/xS?éÇ1I…¡å?©'à2A?'Nr!K?xhCÍ"Ý?ǾS¹'c·?©>Äû¢w/4FGL J1648.7+4834?í9ФÙÏÑ@CúúaZëÀ;mÔZ_ÇçÀ<Õί%@)K'Mð¤@Y{2¦E?Ӟì>Ø
?ÁñÞªïj?ò^/`?Û¸?þüE2º‰?ë{¥BDH.?çaR*o?S¿é!³äžzª¿©š«½]™
¿ç`{~¿ïþÜÇÔUNASNone?ï©+©79z?œÈè¨ñ–Ä?eý½¯Ö")?œ«o4Ï?€5¦F<"?{Fvþ¬ˆš?ïLÈØLz?'Ñ!‰Y><?a­û­@d??nšxˆ¾ë?"I‡oNdK?"y''ˆ?îtq ?''ø±5´?|䛲?l⬗lPõ?«Ü6ۜÇ?j}bÆJ´?î'ýDÐÞ}?•yŸkOÄ?–臣™a1?‹Ò_K	\
?¢çá%g›?0%c—'h4FGL J1649.2-4513c?á¢F·}ú¿Ò¯¹Á'@âÀ8!:жfYÀ9'˜³ÀŒM@šô¥A@ÍãÉª?ÉS–€	¥›?×D¾uñô¥@úúr!…Œ?ô÷öO½¿æÊUŽ§Î?î‰IõíW‡¿äwv#rËÏ¿ì
"¸aþ¿ë*e~ßÙð¿ïÿø]Ê5™UNASNone1FGL J1649.3-4501c8?Á"·ó	?Ñ´üûÏM"?ƒ†U
÷wP?•
ò	Ë?ëPà~e`?њÅØ,æ‡?'"ªn³¬H?—¼,ñ2‹?Ô´à1"ÜE?ȱó¬wU?åê"Àt{?È)ÙÏéš[?­@ŽÛ|k?'#ê²;ý_?ř}o7?¦FBeóà?蜲ìk‹?¨oYoþæŒ?WˆPè?J…ë–¥-Ç?ÅññŽûL`?²¹¾8 ?êw¿"™ '?²Ó«\;ìw4FGL J1649.3-4441?ÆYgÝÅ?¡Uûà
Â&À8š³zoÔÀ:6¥Nفç@xF(XcÄ@'I†\?ÄƞµbLü?ÛÒF‰QLú@Þ¶¿DN?ñ#3¾ÉSñ?ï$'¯ÀM¿ÓÁþ\緊¿ÝF1\ïDF¿ä8Ÿž–Xœ¿ìŸÖjÛ@¿ç,ÉVö†ÚUNASNone3FGL J1650.0-4438c?\Áx0öŒ?V³T"?½͏ éV?ºÆiHAJß?ìQ%'g?ºàÑ3œ`y?‰Ú6®Þ¸?‰È ·1t?ÎôÆeƒ‰?Ä­óZ¥?ç۔4'ã¤?Ä[b_
›Û?§Ñ¦¸*Ë?‰I'¸W½!?Õq›j™Ó?²Ú{t—Ìö?ãÊ!0i?²£Ì°Óí?W(gú‹?GÉ©8½tê?È3Ãøn½?²²È"ÛÑ ?éçNm°~Ë?²ÐÔ¿˜Íö4FGL J1650.9-4420c¿ÒlbÈæÒ÷?£Ú"1`ÔÀ8W-À-À9™™ãktÃ@A0êX£Û@ª¢]yÑ?ÍZ@ãÉ?Ö®F#û²¾@"gÁLf@.Š:ÖëŠ?ï÷õoƒEš¿á^ÛÝáÈ¿â·[ÐKÝ¿è°é¬×d¿ïÿ{@>Ç?ïŽXÐàÙUNASNone<?¡‰ì1 à¨?¸Wï1ê^ª?tpb2m?—Œ!Ò÷$V?îbݙbàb?¹aŸŸ?¦µÛÛ¤1 ?«´Kxòç?²b†Ç''Õ?³Ùôì…Ì?ìHQiS—ê?·¹€Òi
­?µ"åOY
?œgA~v'?ÅôZ=ð"9?¦U¾eFÙ?çÞ¨³ÙïÐ?«èË)(¹?f`rÎíû¸?^2#[]Ú?£'1N'•ú?•ìaƒòŠ?xN˜¥?–`4O4FGL J1651.1-5848¿ïó&äáÀ"Op\‰À:lm¥À<Lï'Êr@eÂõ]¨@`¿B Ž€?ЬbÉù´?æYYø™Ú@l¯c/zA?ý‰oG‹"Ù?é(j¢‹/ɿޘüŸ£I¿à|·áƒ=7¿ïÝEö"V;¿ïøï4Ö¡b¿ëwž!"£‹UNASNone?É=
,?Ã@Td¿u×?Èd•ùHQD?ÁW<…X¡Ó?ã¥K>ª©ã?Èkxþ7Í?Âj•Üž""?Ş'–J!¬?ÓXâ2Ô,m?ÐœÉ]Æ?á¸éonDè?ÏÒº0âÌ?ÎnÑÍ
Φ?¬ÛC,Sh?Ûˍ-Cæm?´‹ª7C¡?Ôý	ì6²??±[…á­š?¶ÿt"ÝÜ?˜Dx3	R?ášýS4¹?·(lÄ/lò?×
(4t{?µtaF¼Þ—4FGL J1651.7-7241¿ÎõøN@«À1§õûmÊÀ;–÷ÎVòÀ<·•XÂ8õ@!MþºÞ?ÿöÊ,œ‡?Ë9\˜q‰¿~6¼ïMð?µW"ðbS?ñå_?ք²?îvŠÖˆ7r¿âì½B–'Ÿ¿ÜÄр»§6¿äM²À²W¿áf—éJ¿Ó®,ƒk¯ÑUNASNone?ï€3¾¨0?†Ù?§žš?Dé««î¥e?@^Œ(a^?Ž±XU—	"?†r䍵4è?ínÅ*'XN?»…ÿ>²ë7?€µ˜èžª?"¤`×bk?²s#'±hL?º €"pç?í΢±_Ì?'t…tð½?wkJz8S·?mûµ$HD?°^BÑ|e?y—gù~·?äîÀèÒÂ?³_|´/ˆ?–$7l¶—?-TdÊ?ÔÀ:½£°_?´~3ÌhY~4FGL J1651.7-4359¿ã-íÞDÈ?ÃsÖuB!À8Él4Á
À:?u –
@†«×‰¿1@÷n¾ú|3?̂®›‰]â?ãD:AšT*@³Bؤ@8…a8ª?ïü7ž|ØC¿×)íÍ:¿Öª9DDR•¿æ%Ž?w4¿îrg'Ñ`¿ïÿšÜ|UNASNone?eAE®v‹û?^¶ºÊ'5?Çf âµúM?˄ŽÌDµ?ê6¤
á?Ë{Ûá#'?!탆(?"l.%^±R?Áó|:ê?½9œÈ¹Þô?ëAþ­;q­?½;4˜»Ù??¥™ÿۂ1?†¾úÄ­"®?×àƒE¹®?µ¹Ü¤'?⾄½%y?µ
.ßh5­?`kÜÄ"|V?P	¢|WÊè?·°@Ø5ê?«¦üÆ×{?ëA¨Ð	?«ÝÒp'°4FGL J1652.2-4633e?î­»×~xù¿ø¤ˆxßæÀ6ÿÓÚÞˆÀ:4
*%mx@!?%Ó¤,p?þ»Q•	Ö?žBSŒšÉ?˜€k˜¬p?øþiâò¨ÿ?û~"æ+˜Š?É¡î&ä›K¿Ñ(›@¸­¿Þ•ƒÑF¿ÜIøœ‰c¿á–2§9¿Ûdÿ§j"UNASNone3FGL J1650.3-4600?°}HþgUš?§ÎÐß
yl?tó7Q?y½{_1<Ç?íÆpqÜ?©KÜ
t ?ºbP€/ú+?½Öp¶)Ž?¼cê=f?Â|œÖðt?é'S|¹
?Åhª%c?´mAoB˜¶?žÙòei$°?¤KöWâô?Õ¢…¢?ì0Ó².¹?¡›Ï=§$?±$ßz? ºVùSF?ÂL€æª
?°s}‡d6}?é:Ê;Eù?²:±³HNp4FGL J1652.2-4516?҃a_|£{¿ç—MYO&¯À8¶lCõùÀ:GHÕ[ç‡@Ø èØÇ@¯ð£kªs?ƏêÄ.˜š?אջ2ño@'ö@c^@Ç&)àN4¿ë.ñºÂß
?Ɓkdýێ¿á)à¾ò·¿éA 'oÿl¿ìàD]ýâ¿ïû.¡UÑUNASNone?|ÇJ=ñ€?r.ºJÿ?²¯_rم?²åëGB7-?í"•Â˜?³;ºD`îã?žä°,'Îè?›@‹²??ÂÑBѹí7?ºkËQ?êT‰Ê,î:?ºÑÈáZ1î?­:gK"A?‡GØà]·(?ǖu7*C˜?§ÙXõ/§Ü?èF¼=|>&?¨¢ó9Gvƒ?ŒˆÅrrƒI?u8ª˜,T?¾Û»2½¼ž?¢^H§T`©?ë²eƒÞ~_?£(¬5~ÎI4FGL J1653.0+3640¿ïùÀ
ï@CW‹'¡¡À;¦±RFÀ<ÿ>Dß-"@Á¼.™ñX?ïö¶À›æü?àã¦Î5'™?ïöÌR֒@Šc0Q¤@~¼èS;¿åf3:¿ïo¿ì©õ÷¼e¿´3'J댿Ç–ý]
w¿ïüÙ¿úVs¿ïð²…"êUNASNone?í:šbzÀe?À:OböÔ0?™\Y¾?
ý«‹"?²8Xˆ›?¿÷aKX$S?ê׸^˜?ÀÌ5ÌGùW?­+¯ÐB?µ»'€
h.?º¬c+Ħ?´Ãu¸í*˜?鳸FÓH?©ß>v;€?®ˆÆ"öT?—äÊýáuF?ÁŽíí§,L?¤ë°KzC?æ˪\'R?¸ªÇÂ.¶‡?CWL½º ? "7æÏ8?Дvz{Õº?¸/r¹jÒ4FGL J1653.2-4349¿éØ©H}2?­‹ÛàùïÀ7œƒujæ(À9Žß‰gó.@@éTA÷@=¼>	P?¹{'G•Á?Ҁ¿®Xë@´û'Ã@æb I?ïþ'ÍzÈ?ãm¬átú~¿å—˜mI¯v¿çךÈÙ"¿ì'†!퐒¿ïÿ踻ÐUNASNone3FGL J1652.8-4351?'mÞ1…>î?—°æ@ñaÈ?Û³K]"No?ÏBÖ+,ž?áܢبÃÍ?Ï7ÓV–Ž.?z'9˜Šu"?"FÜÁ–Ó?á"õ¹¢öh?ÊÜöpyàâ?ÝQw¦WéW?ÊËj¿n?£$´ÚîŸW?'¹¿ŸüX?Ú´Yð$õy?»^;±_?ás‡º>›N?»D£öL'Õ?=§¥Ž¤?/¸Ž-éò»?Õb'9iè?µQß;v?åK7VZ?µS-Äű4FGL J1654.2-4907c?µÒ	ú4!
Àe¦$ÂW(À9ŽX«'ÀbÀ;8òòÑCT@ÉÅjØ»î@ˆ¸»Ð`?Ç>ž¡@?Ä÷£‡?û˜…+•°@ !ÂG³¿çíeÿ8Yä¿èÛ­À˜$¿ç]Å]l¡¿ã¿FÒLhŽ¿ëe#ÀÏhˆ¿á¬åÁX¨UNASNone3FGL J1654.3-4907"?Ø (bÍÞ?Çt?'Ž²Dê±Ð?¥±~PÁ?ã#v<×Ã?Ã;Z¹‰G?Ûè@ç`3?ÇzgӏR?}åÚ4™µ?‰¾–B??áÐ×æÆ/?Ç<ðck¡™?â3zíõ´?µIÒttd?§‡#mŒØe?''+<Ÿke?ب''ry‹?³\¥y?á[pl^^?°y̪ÛЫ?"‰rÔrŒ²?@¾A?܇ú˜x?°s2034FGL J1654.5-5509?ïÛ¦"ÃÀòFà!qÀ:6ž«QRÀ;˜14@î—\R'G@Ž÷!4-.?ÔU#}³Š?îÒ/w¼Ð@å?À	oë@ĆD}2†¿ßÇ7a–
¿ÙVÁãd¾Æ¿îˆ™A/R¿Ø8ÄA¸Ý¿î?²{è¯?äÝC!½¿êUNASNone?³àco¯?²ô'o>Ë?Æא¢;"?÷ŸUÑw?çÎu{T?Ç[•œ­¿?ËxqÙRÇ?ÉÅõ˜@?ӑa²¿Ü]?Ï㶩È×ÿ?Þ²e¿Sz??К?ÓZ¢»ÑâÆ?ªÚ‰¢oÙ ?É¥$?©p"A¼7—?à
í8³E—?®;4íP­Ü?ÉÅ¥s<?¹Q7I?ÞÌ)˜ˆCð?ÆÉÃ2
·8?ÔQ§±s?À¿^¥É~±4FGL J1655.5-4737e?ïj"êÏ°òÀ@xw
À8Ý/n'"šÀ:ö´°¨ª@ €üU¦z©@¬ŒUÜ?¸.ðƒ`G>?'
ÛéË5?ÝüÙ·–Û@|²>¬
:?êؕ›^–¿×þí›ÏSæ¿éÖt`¿à¦"Àä¿Ý@€Cdô¿ä2Wk!UNASNone3FGL J1655.5-4748?؈¨0ƒÉœ?ÂÎ="{§–?}ȼŠ
½'?sÞQÊëÚÍ?ã€n©ÿ¶?Â×:-´á<?Û¥šT†?ÈjK±?tú)1€ÿî?…ål d!?â>ƒYøw?ÈQyG&¨F?ÎùcvKˆ?¬PS:¦æ¬?­.T⇯ï?'¯¥þ¹ª¶?ænÁÔD¡Ÿ?¬¼µ»¹?×¼œÒê×Û?±G2úÁrè?žû^ŋ‹?‡Î{-CÍ(?ã)Ö ^;6?±U/NÍLÞ4FGL J1655.7-2411?뇚<4@'ºYÀe¶=À:mˆXÿvÀ;áÐ>qT×@†+<™¹O@GE‹$Œ?ÒÌÌ¡Ù¯?Ñ}	@¢C@kõQPT¬?ñÙ5©Eµ?ïþ;9'ò?©2­ý(à¿éYe5
ÿ¿Ø—9¢¸ý¿ïÿë""i·?ïúY,ÁÿêUNASNone?çìcUM?ÃË¡Ñ`L"?ž_ÓO6 ?¡ŒK™{O?́ÈÅÏ?Õulw?âRxT…ª?ÏV¡!1"J?Ä£²Pí¢D?År³cDzÀ?Ñ	6.
‰?É?G<êVv?⣴¬ºs'?®ã_`àW?Áľz¸Å?¢`ÚtÁè?Ò04GM¼z?©€2{ñë?Þ%ƒAíºª?·X½Ð<?Ár‡B4R?°
ujz+?Ù!9ø:­?·¾R9u4FGL J1655.9-3940?ï0úÀYŒ@@®I#`À9oe5
ÿÀ;
w?Ò}ç@Dl›ßš@ۉC
@Ì?Í58[' N?Ԟ$c½ù@%XdE#ö?ûqo´Bè2¿ßÒËÿÈLµ?輸dÉ®4?ÓS]Æ.οæ7ûþé¿ç®¤"‰—Ä¿çºßr#UNASNone?°Wøé-âm?¤kS	?¤[[{­Úå?¥U*ÑJ¬Ÿ?ì¯K+f?°ï%uÿÃ?Á£×?¼àš
Lß?ÉZ*0Ê©?ÅùÊËnå?åd•¯3$_?ÈV‡=ó–?Ã	ÏGZ"?Ÿè"'ê"?Â_r®Ûþ?¤>A(
K?楤Ñ}¤B?ª®á<CZz?Åòu«¢šÃ?¨ì£åρ?Æ$?<:?u?µ"T ¤r?äúRÆÉs?¸§í{×âÕ4FGL J1655.9-3101??þ6–@šºŸ¹À9óëƍ«À;•ËWÇ@Ë…$@22'3K‡?Êáž@zµ?Òa]¿îî@YP%²A0@ûÅÜ¿ì]ä·¥?ï¹ý‡»¢¿æ!;¹êqù¿çlÁÊ:K¿é|0¿ïø0þ¥ŒíUNASNone?ÎRû?¿aK€«] ?°Ãž©8ö©?ª57Âg?æe†–S^-?Áíg"Úø¨?ÙSÄdç?Êl5–n?Ä<÷¨ËÁ?ÀÌ
F2J ?܍À†¸?ÉÞØŽ8/?Ô}ðªdÁª?«öOº0\?Á<û€AP? 'V³Š<?ár+íŽ×?¬º¨ø´7S?Ýnæ%Ká{?«)~P‡NÆ?Å,<I)ò?§æ›	'Y?×úûΉ?«\ÆT™½ 4FGL J1656.4-0410¿çÎg­Ÿq0@7.¡ ÏÀ:µ¼åÎüÀ<Š
RiY`@c
ÔoX}?þÛ£"Ń?Ì­3ªQx?ä) öÍ1@X§ç:6]@+C&E?ïÿ0,µÿ¿ç9Ù	ññJ¿œ9ÄØó²Ñ¿âž€ô‡%ú¿ëS—tü+¿ïü½àö¥cUNASNone?Ü#l‡àÿ?Å·­ãŽöj?Ûû‰Lö'"?ǝ~T֙?¿"(¬¡ùo?´wýÄm?Ù˜Ê;?Ì¥?¿z9?Üž=ØÏ5?ωáßW¯&?Ãï"sÍ?·×âN*?א><{G ?·K5ºÄÄ?Ü®TșÝ?¸ù¤Œž/?ǂÛwx=?¥b4u#É?ÒõÞðÓþ½?«|¦bw†Ú?×sXv8Ñ?´ä(×é?Õï­¶µÈq?°87ŒßK4FGL J1656.5-2733¿ïÿúÉVÂý@#Zï
å6PÀ:ŽP±É;HÀ<pSó.@ªvºœs"@kXZ4?ÍOʘ•Â?éäjþ{›'@4,ºËC@·dÒ<£I?ïÿ0ýñˆ¿è‡¤Ú?|¿³çÆÎ0$5¿ç¬—7¿‰î¿ïÿàŽ¾¿ï±g¸ÎéUNASNone?º~…"§
?¶+æPð?Úӏ8Gú?ÈÒ¤Þ³Þ?ßN‹,C?ɲ-0w[?·ñ~î?Â?Áz°Â{!?å¬!R^üÿ?́"ý1?ÍV»?d}¥?Å»ôÔ¼Ò?ÅeÌÍ_­ÿ?¦ÜKßZÄ?ãº%o<q²?°ÒžÜ'K?˱u®‹7?¨Xª>rï&?¦0ç¤;'?Õԟ‰J?çÚ,ηm?´¿ö?‰Üñ?Ë™c¶>?³Ñlɯ­4FGL J1656.9-4814?ëÌÞvÝçÀ	½nŠø'À9Ã;òõU'À;[;¸Ìe@UM–
îÆ@vßîÁ?Ö;Y½‹'C?ïNÀøƒ3ý@	 Vßà¥È@‹~M㸢¿ë}	@¢C¿ËßýV,‡r¿ç%IÑiò¿éŸ}ß(ïã¿â+úú݁P¿ïò¾UNASNone?Àñg£^þÉ?¹¥_
¹×e?¨?…hzª(?¦dW@
 ?ê?­À •«?¾vÄþ–`¿?ÇO`¿ºd?ÄÅHP¯wm?ÁešŸ.s"?Â+QøZ?åÒÕÀtž?Éð»ÇjF?Ò5±¶h~\?®8… Æ'?Á†4–ê?¢;ä_Ó…?⃃W¦1?°ù0úÒt¼?Î1ïðÛº?³ã ®*8}?ÒOÝÍ:"Ó?¾7ÊBun?Þ®‰:Í
Q?¼GðjÂ4FGL J1656.9-5717?ǾHoÛZ.À!¤Œ?>qÀ:¬TƒåÓ.À<+óV¤Q"@=lè5³ì@ij­?ÑAǀ\±²?âȘ?|l¸@,ûõ@þè'¯q¿ï¾´ -œñ?ïï* ­Ò¿âî1× ì¿éHÂ:¢"¿ìŽöþN¤ÿ¿ïÿ¦¶tFUNASNone?Æ8=糧w?ºC>ƒË}?Ñ3ïpSJ4?Çéq"ñ)?á×øÍéq?Çc´^k"?ÙOjƓ¹
?ÌLšÄ&ð?¿ ¨Îú?¼²· [vò?Þè•8ˆu?ͨ¼æ\k?ßێ\U??µ'GK-¤F?Ï9qƒëÆ]?³qü\TP?ÑFk¯­Ç'?©4ÂèÊñð?â~,­ûã?ª"Õ@@Џ?ÇbÓW"Z?¦«±FAë?Î¥LxL|?¦ÝÂn)"4FGL J1657.3-6232?èç"oL$WÀ(+{®ÍÀ:jª|?ìÀ;Ódύqm@^BT8fy@œ÷_GŽ4?Ê{mI.!?¶XYÞBÀð?êÂä`è">@•¤"^¥¿ïüÏ(ǟf?Ödü¿â	€²B¿æ™Y_ç¿éßv½Ì~É¿ë{j=‹|UNASNone?ì|DÕÂ<?¶ZaRå?–ݲ³`lz?"_Ö
ó/?¶ha,yÒþ?´Sӗ-7]?îÅS¯ îy?¤Xÿ‡"/?b·'inÙ?rLÔÁȲ?¢}ܓz?£Ž)½ª:?ç_™u?¯¶¥™è"?¦á=nŸY?v\£°?Íó'ó%òY?¬Ïm/ü?êèõ¾Ì;é?Ÿûã›k€¶?–³Q
*/?"7~/D¼?Á…¾ãŒË?î!o嗖4FGL J1657.4-3917c?îÿ°­îv|@TÔ#&vÀ:_©³ÃÀ;ŽÚLè@Ç)_Iç€@±'!ûÓK?Ð
CàT"?á¡b§K3@	· QºÞ?úÖ=3'(·?ïùh6J>连à7|‡Ôº¿âYl¸K¿åßbцoñ¿æÃ^)+¿ïÞ´ -œñUNASNone3FGL J1656.9-3919c8?À¡	/|ƒ?ÊéìCì7O?¤X±Õ.;¢?¥G_ˆw‡?ê'2–Φ?ʜ²É_V,?ÁDl±0?ÁûŸ#Šð?ÇV¯j‡ô?ÂÈø­: ?åÙ8ùýž?ÈãLšC?ÊêU?¥z#]A(]?Ãϓ°j?¢–§)Žž\?äv×Lõá?¬â¢2J³w?½@»}ÛÃç?˜duTÒ\?Ё׸
û[?¯
ó80?äü´=‰Õ?°Z—¼‰"õ4FGL J1657.7-4656c?ê¢
L™·À&"»À9$¯öÓ0"À:̨¡tYn@X=EZÓ
@ÿb›ÖŠ¼?Å3{''PÓ?ÀG/~ó¦?þÙ&ýšÊò?üÀ¤ ]Øù?ïß:Þ"_¦?ê÷Û8 Z~¿Ù™»þHoÛ¿çWšPx¾X¿ßÑÃ×/Ò¿ì*© öUNASNone3FGL J1657.6-4653 ?­=Ì^6-?¤ŒW›‰mJ?˜	L¢¹Ú?–Ôˆ¡2Ð?íkå$MÍ?ªWT‡¹?ÂäKìTëÛ?¸j—?¦HÊ9ƒƒø?®l5º?éâ`aRŒÊ?¼­$o—Ï?­z"*vH?¡±²D`-?¶ˆ†Hœ'[?ƒÉõ>vž?胐®a݂?¦@<É+e?Àþî&w?¤©tjuu?¸rÊÕå8¬?¥.kp%q0?è²i¹ØM?¯6`–I64FGL J1657.7-4520¿ÑRPæ~¿øsÓ¼«šÀ9>0vÀP¾À:´ç]7@ \oço@ÿ¾¹ä'¼?Å9ügÅ?´»1CïÃó?ìr9¾g¯<@%e/.Á´?ï	Zò"Ý¿ëݟM7Á7¿Ív߇ϿçXࡕç]¿êÂìÿr;‡¿¸Ï¾Ä¡Z-UNASNone?TH÷'o?'¸ä™ºd?"#^ˆI8Í?">‡¤q"`?îtBÄ%V?Ÿl¢Ö –?ÂE‹ÈÂK?¹³eÄ$·á?"#¾UÁ4?'öç³Çl?ë(~Ö")?¹·qy\ó7?Æç{xÝ$?¥®®ó˜í?´´_H?"æ_÷n"'?çÃ>ë<Ñ7?¦†5×JÐ?¸›Y1
º?2þF1L?"³Ɇ?'èß9žƒ½?ìHœ'w?žñ"Ï2l4FGL J1658.3-4637c?ä͵ˆ–ÀDoÞµ,À9Zgä맃À:×qºWC@ Ÿê§Ê@‹˜AªÅ;?Çð½Ø=CW?»`õ
]¶"?÷­íCdٞ?ö¦+'Ëöä¿ïþ°nÈ5?ïþ`ù?Ÿ¿èýIúÑÿÛÄQ¾Ž›¿ëüº0ƒ¿áü\§ ÃZUNASNone$?°»TIÁY?©œ®.äù?›‰Œ9ŒZ?Ÿ­s5fu8?í*fy?°vú'(è8?¹'¨­?¶Ý2±uR?¶íGeÍu?½È{?éð3¾G/?ÁîPÃ}۔?Æé1þž?¤… ž‹­ö?»(ÕÕüe?  ônÙ¼?æàžEÀL?¨Ñ<ù!î»?´)cމOG?—H
Œ–k?¾ÁA,p«f?©å&øh?颫^ À«?«ì¬PÃ4FGL J1658.5+4315?áè–Ž*@C#£ÂÀ;å§Ð"ªÀ<ý»9ýQÐ@!Ѐ2ë9Ê?ÿB0[è^#?Éq*º"º2¿¯ðZà:+º?à±&~
"@ßÀÅW†¿éeì"ÓiŸ¿ïî>ÅèW?ë	IàsÈ¥¿åMtýØÞ¿Ùd^—ºò?ʔG_ºû"UNASNone?ï#"¨ò—Q?˜›npðl9?Sg•
6Ö?P4|ÜÇc?še1'	´w?˜R€á0X?ï*kü6? çÊ:læ?a%2Ýí?sR}…ÌÓÍ?Ö	|}q?Ÿ{/±8'?í´03‡N\?"¥îxQ—?vÔc§W‡?i'"W¬µ/?°ý‹¢?'È&ùÓG9?î'M'c·Ä?–G×*d?X5ª%'hÎ?[/è–ð–?¦)y˜›H?•÷xrÛ4FGL J1659.0-0140?Ø_ŸðL@7큾±À:»df²À;ÛVSÉ«°@6ÖS3XÈ?ý«m6d@?Ə¿P7{?Û¬D6¿@a¸¼-B?÷ÚJ><¦¤?ï ÊæB¿˜¿Ý ="(¿ÍÄüžÌ‰[¿à^ý':пïû½ü?ìôêÃùUNASNone3FGL J1659.0-0142?É°KËë?¾*pãgó~?àó_8é
f?ɜÞAŠƒ?ÑA¨¤ï¯?Ä%Ô1º¾N?ÑÐçJµðU?Î3±k-˜?âòtêÿñ?Ñ)4ë¦?À"]Â8"?¶C
œ(½ý?ÊÞ'YKs"?®kRÅ­(œ?à\ ;.¹î?·ÂG}Ä?Ñ׫ÜüÒZ?¯V'nâ?ÆrBy'?¨r†fà…?Ðef52Ù?¶‰TÇ~Æ?âEpTȯo?ºg¿ÀªV4FGL J1659.2-1443?î°¥¢™ûó@0ÉõœÏ®ÿÀ9úú0³&3À;ڻݑ@/@ô%ø¸
"@‹Ù½v?Ȉ}£–s?Ó^lÇÔ@} >ÏI@—†¡ð*J?ïýW¿.©Œ?ÐëÂßä¿äTŒÿØ<í¿Ùª‡Þ0Ly¿ï['\¼?åF>QÊMUNASNone?èè`@¿&?ÀÈv‡ÿ?¬'‰•Hȇ?ª^Fd"?Å=ܗ±5y?½/™u|?ë$#Ï;¸?¾PR-›"?­iY7dŸÙ?µfŸÞ@
?µB2EÓÒS?°	«e]ìç?䃎¥Ò?°'a"i3Û?¾…•f?¡ñœoÜG?Î¥ú儈?ªÊn…Ê?蒢¥Š¸¢?©Aw¼°™?´'Sqªà? në.0uÔ?á˰ÿÕ
?£¢¼4mÆ4FGL J1659.6+4918?ìém,B@CpޏlðÀ;§iϧr À<ßjT1°|@"yÅï@ÿÿ«Fj?ÓZ]āNÊ?¼.)‰_?æ×
˜n÷/@œ=D:¿íèØÁ¢¢,¿åP³a@➿àz=|bQ¿àœýÒ(V¿ßå»[5ZÖ¿ïý(_D´UNASNone?ï¼·ƒ@ZÎ?}K«e5C?BÿyXÑðF?=Ÿ<ÎQy?DO4¸[=?|‹[G&®Ñ?ï]¾Ò>¶?'x÷/4ÔN?Lþl!/?XT!N£bÉ?"gý̗˜?ß&°(ö??î'¥™ëN?'OŽí1?vÚ.»!?k†Óßv??ªª`‰æö?½óØµ?ï7
1my?'™EE?V&uE³³?LáÈ°*å'?—»ò~µ²?'}º@f4FGL J1700.0-0122?ç@h¼h6Ü@7ÝxqOÎÀ:oSשÀ;Ä76Íòg@Aº£@°'w"Œ?ԗg›ñ
?ãÁ1"·ºí@
çööl@ys×=>$?æA-ô/?ä˜`‰' ¿á…²œøŸ¿ë¥<e¿íÁ¼-BXj¿ïþ/EgéUNASNone?¼–ÔbÇf?³ïïnû?èÙ×0´–ÿ?Á^&]jÍq?¼šrZø€ž?·Ò°¸NŠå?ÒN©âµØ?ϰҒ¯A8?âé˝½zd?ÒTXê•]˜?¿vû‡<̍?¶õ͚."©?Ô^Ùp¸½Â?®§(mö	"?ӕÛéí.ò?°ì–BV"þ?ØJ¥ZN?¯$Zj'õ?²žKö?•hq­NX?ä–zÐve#?ºí"g*±?ÒR¢ÌQî¼?¸à×î¿ii4FGL J1700.2-4237c¿Ü»­ù€'•¿É=4D«+À8N>X*cÀ9ñ²½W@–ë_µ@G`Æu?ǹNè›_?ÜnÛëMÁT@d öðŒÅ@ˆŒxô³q¿êâ‹`òË?ïüJ~Sm¿å-݈ܳ¿ì Ñ0à¿ïÂã>ÿ¿ïö'=¯¸ëUNASNone,?ƒóŸPhÀJ?…¸iø{³? Ö»ŽõÐÍ?¥Á'\§Kü?î¢ÅÉÎÿò?¨¨îð‹¶?›ÔöÄG¢? …&Vð±'?ÖùW¿­·d?ÇÖÓdâtÕ?㤬jë™?ǏP_ `ž?±Îú;*ê—?"#w3g?Ňâm²/?¦³éÜdR?èd(7?6!?©¢6ÂØ?}i¥²b÷Ö?j.¼ÔÊYq?ÌìjgUÊ?´¬úéî?è¿1šdž?´gœÝ€Ì4FGL J1700.3-4557¿²(õ̯ÀyãìëÀ9&p­FÀ:ŠšÔ,<Ÿ@ÐÁ{µØê@#Ɔa®q?ʘÜñç?πåÇFü@c›{)Q@¶•bþ'
¿å‰¡iq³¢?ï†Nc:aü¿æüÚQοæjqáÕ¿ê4{'W]µ¿ïþêÁªYÛUNASNone?ÌË|9?¹Œ°ÙB@?Èp<:ñ! ?¾Ëu¯ÀF?âá¾?rJ?Ã~`š}Ó®?¼9ß±ð¿?¶ÔsáõŠU?´î®´H?µ•vÊOØV?éÛM‡æ?¿kIðm¸?ÄO‰Mw?¤.Aµî?Âð9ÂS?£?p"ÒÎ?æ0ÞI
X?ª"èUÕ÷?³
3_IK?"³
(WÆâ?¹ìŒ‡^å?ŸŠ™³Ýú?ê^»¨*ú?¢pƒ@|š4FGL J1700.4-2746¿î%Ÿßtð@!¼—ú](ÐÀ:C	^M"1À;¸+`ÖÚm@N'·ވ@L'Iñ?Çݏ'¯›?°›»\âÙÿ?æ{—P=Ê?úQÕøÅy?¤; :XÓ?Øß-jä%¿ëàz©"¿ßþè(¿ãƒHõ<X¿àҍÖí·ÿUNASNone?Ó¨´•ß?À¤õK÷ïA?"BÔùñw
?aò¹?å×ýåíØ?Á)~jÐ{?ã÷µz¶Š?ʚmTÎ?˜ä˜‰²&T?¤gã
?ւK÷ȟ?ÉÛ&#OÊÈ?àðà°:'œ?²	ÐߎR2?ªôc$Ÿ%?'õì\"3?Ú¿²;(ã?±¸D±M?æ@¨ã}Ð;?®áæƓp‹?¡D­øe™?ŠKføx?ÑV,#ER×?®ÃF—ôO4FGL J1700.8-5218¿ïG›qNæ‡Àßþó…õÀ9ØU)þKÀ;uÌ¥_ z@bQãÍo_@ãVg?ÏÚû#L`V?Ïud8#2@â˜E܃#@×;Ëz?ÖÊ¡¤U	r¿ë•X¢žÁ¿çn¿0,¶¿æùÄaÄ@6¿ïþùoÃz¿ÔÓ@h¥ÜUNASNone3FGL J1701.3-5216?Ö$ÿ¼Í?Â0?+¨m?¡bˆԘ#?•öQV)‹?ã×W¡Oî?Âtã)9ê?Ðÿ$Ì1»A?ÂçyÌû??›%üüÕ? 5¾??æ§=²qÁ?Ã2"ˆmo?×ÊIу"×?°I-#Žüg?ºÑ)Vü:ƒ?™bRGM#?àÀµì^®Å?®ÒYm1at?ÕÖÈQqé?­;ݺýҐ?ª‡¹÷   ?'g«ÜÔfÕ?ãl 8½	?®‰Î­Ä"Ç4FGL J1700.8-7304¿Äʍ֏pÀ2jázû]À:ÿȘŠ¥áÀ<w7ð1Uã@VÔ}›6@jÕ`ðà?ß{2{R[Â?à!ï^G3@vn¡žJÙ@[<'¦?ÜëÂFa
?æ÷©OBÇ¿à.Ìț¿çÐÉ{ßto¿åÕN±=û
¿ïæïÝ ,UNASNone?í˜ïfþT?ªfzXäoŽ?‰ƒË²Vú²?‡ÝW4nfR?°U5.?¨c4)ʛÓ?îúCì^‹?§O®Äã?W?ÍM"ªGˆ?çï'HÝ"?¤²ÄÎb?¢á'ØÙÎ?ìÑî²+?Ÿìؽúç?ž€½-"7;?ŒÚj""Ÿ?³wŠ%)`Õ?˜z	|£pò?íRð	Obø?–¿øJÀƝ?'ìÏÂA?|ÍÛ·Ü6?³'ÂŒ ?–*ÅBe³4FGL J1701.3-4924?á¾}9ø°À
2±-4À9Á.^¸<À;=¥."R:@JÀ¾ ·†@ Uûµ¤?ÏÊ,–?Ò,¬{ž†é@:ry\ã?þ<«tp–¿ïþÐW›È?ïý‡ŸñøU¿çÎÇ]øÛ¿å§û'Ü5ö¿ïþ'ö ?â²aFkõUNASNone3FGL J1701.1-4930?ßkäýÛ×?ą"žH?¼>ÀOýs?´˜ß(?ÙêäâÍ?ÄîNH!oF?Ä|(@ùÁ?Àj5øË"?Â%Fgž^?ÁTnE#{Æ?æW¤UÚ18?Åò‡€®í8?ÉÁüu@"?§@ÇB*RN?Ãr³«¹"+?£<jJu;?ä²Ó÷Áyï?¬êøÔۈ?Æ1oVýs?¥+É	_Ž?ÎbyùL?µc,É,(?âÛ«ü9Ñ?µtþ,I74FGL J1701.9-4625?Á"^¡‰¬À7´·,À9¨3ša?¶À:Ûd53¾s@/©Ì—Á@¥æ¼b~?Ðkj|uœd?àR=à
l@@
?:¬¤8@´™Æ»á¿ÖW}ë=P¿èÏ"Îš¿àôG/iz¿ê2þº…¢¿î?.Ö­ ¿ïSÅ¿½DÅUNASNone3FGL J1702.1-4623?°'mü¤ª?¤®úÆt{§?ה´?]D?Éz:-'L?â0¸5KÐI?Ê{zïy?¶Øûy‡H?·9·fÊ÷?·gê…sè?¸ÀIv^Z
?ê7ãKÂR?¾O¹¬fÄ?¾¨ç•)?š
z¡'˜%?ÅBõŪ1?£"ÖÌÎûß?æìí Ûóï?¨U/ŒÚ?E"‡"?xßþ"K¯?ÇîÎȳa‹?².Œõ@ê;?é'#9›™?²RЂÉ54FGL J1702.0-3721¿æIeqca@+xÚq3À9¦Å¿'Q§À;vy!@ûÝÜ@MÅ2¥?ËbV6mzW?Ð ´«m×t@ZÆ3¡î@ZªBß"»?ï±ï,»J¿´{ƒ"…F¿Û»âï£ç¿ã´U'¿êS±Þ3ý^¿ðUNASNone?Çt%\]aÛ?·îçf&ܛ?±
ÀÏÇ´?¬NW±²,?è>Žï±?¼ÃӂçÃh?Ô¸¼5J¾?Ç)ðvi?³ç]D³­ñ?·­ä±r®?ã'yNäã?ÈUøEÌÛ?Ð5àǐƒ/?­
~'e&?ÂQ]AYG‰?¢Báã©6á?ãP¸Kál†?®\õ
¨O?Ì­7fÇ)?«;è3¬N?¬˜w*¸Þá?'ØÍ=¯G?ç4¿zÀH?®§ÛvXÿ4FGL J1702.3-2525?êÍ®‰s@#à#éêÀ:9êØPÀ<Ğ*"@²Wz>ý?þý@´%?È`hàê*?ÒUûŸž@à•äÙ3
?ùàçß!ä?êý"à¤ðæ¿è¬ÍT¤?ÐCCrE˜¿ÙØŒ'Á¿å³I€C‡¿ðUNASNone3FGL J1702.1-2524?ܶ€˜¯à?ÆöbD_±‰?œ–âÎõæo?—Ng³)f?àÀ0ÊÝ?Ç|™"mŒ?ÖL§í9±u?Êthv#8ÿ?´èð­²»?¶|Éf¥F?â<©KMpï?Ê0/æ÷î<?ãkJ[Ö?¯*
݌Ær?¸ˆ{"0B?ž£Zë2?ÓM(ºD?©0'^?Þ'ÿÞò ?®ƒû©Âþà?¹ü	Êñ§œ?£Û߯z[?Ûikd£z?±~ÔËð$4FGL J1702.5-4803?ïO±"®RÀÅS[ǦóÀ9»[>À:曶ªK™@¸HýÏ@Á`Dä5Ÿ?Ý©Ga"mÛ?ǒ&>?÷1Me
 Ò?ûæ6mÐ=¿íöÞï@5?ïõuüŸ¿ê¿Õ£5#οéJ>xᓿå¦ÿéYËM¿ê¶iLUNASNone?â;‡ÿäô?Ç?ëå$ÖV?·;¬üL?¶¡˜e|x?Õº/Ü7?Ç°el'ò?Ɲ®‰º?Á¨&ÆQÍ?©…~˜èã?±‰¶¹ÇÖL?èÀ<t?mD?±!ÈÌ0,?ÉfªÑ"F?¦" ô½Q'?Ác×3Ìt¦?¦iûz ð?åcpˆXÅ?­#¥½?ÄÜwïU[q?¨¹Ñ{Þ_?±
ÍÑ5Ô?ªÎøÐS?览J¢h?³T"³€Õ•4FGL J1702.7-5655?ê(Ï|ªuŠÀ"u?À	oëÀ8BÃEdŽÀ;EeìÃã@{¯xÓü@ÖÔ=–?¤¶Pð?Òò1ÀíE"@'ÞSó@/;Ÿheš?ïÌ
ÑyÛ¿Øm-_´›~¿å\iànj¿è¨ujhS¿í†ý )Uº¿åxYã¡$¨UNASNone3FGL J1702.8-5656?–'_Ø(¸²?™Û´'ò½?ëz×YÛ?ºÛÊÈÎä?¾ŠéO-þ?¶Ý-Âgõ ?Œw$¨ç†R?"µX$`°?ë,«â/#
?ÁEŠ'&?Á…Þ,´ûd?À›î'þÇ;?½IÍ:w??¦'xÒ\?æ¸×}õ`ì?±qÄ	Ç|?Æw»{@¶?¨êJx8<?nJùt#3?]¢þ9#?ì%ýÕR¥?£̝Žr?½Ý¿Í´Q=?¢ï*4â•74FGL J1703.6-2850¿ïê*
D·@¨E/‡­À:@€#À<8¸®1×@ Àåä@Ó~9Á®?ôæç€,`?؟ND0±y@=®ˆ*Ü@o¬.œ Š¿ï"ôÁ?ïU"âOÀÞ¿ÒU,«¶¨¿åÜ_ag¿ì´¡mM‹¿ïÿû-2h2UNASNone3FGL J1703.6-2850?ÚS6¾Üž?ՙ3R8º?Õ¯•£‰_?ÄÔ`I֚4?Ïú–Koˆ£?¾{UîúTÇ?âÓáÖ5Y?Íëd7'J¼?ÅMdÊçÙ?Ä;«3«¤?Ïcݳª?Æ¿LÅçfO?ԅŒ¿â¶"?´¯cóž}?Ý8>ÍuÁ¥?¸ƒÕDJ}ê?̄håO®?«‹<Xç‹?ã[ÍXm?¬‰ÑþÎ$Ø?Ę#e@5?§5w™»N?Íø¶|)j?¦('›4FGL J1704.8-4030?ïŒßÅß?Û@¬B"£`À8yÓ3[AÀ:LèÁõÙ6@Kû+/@äÍt'y?»¸€®­?Ôñ[!ŽÆ@Œ[J©q~@y2 ?ï֘Þ2и¿Ì,gç𿛿φ\¥óD0¿ä³¼ZŽÂ¿éÚQÎ_¿ïÿÿ" 5•UNASNone?¢®GÝ9¤p?™Ï{~~Ïù?௞­x–"?ÉÔ>î.?ÜJù©gŸ.?Éww0€šù?–Œw™ôؓ?š>û
'}?ÊM'.Ø
R?Âð3êj(F?è¸RwzUç?ÃFW³ü'Ì?¯«=¶³Yž?š¥ÛØeóe?ߗñ"O?¸¥ôcÕ²?Ür§2~?¶ëLƒaæH?Š†D2DPé?uÊÂÕÑ?Äo¤rnº]?­ƒ
P®/?êyýқ@%?®¬+(j4FGL J1704.9-4303¿Ñ"Ý ÷S¿ò'U^×%ìÀ9a@®Eù	À:‰q€Ø@ %ù	@Æo@SjZç­#?Õ¥dd®€?꺪ùš‹@2&ù'Ô@í‡@¬n?ïÊ4f?êVžrFny¿ÙÇU¿z(æ¿âuÂú»ó¿îÒ¾©HŽ¿ï¸fC*÷ûUNASNone?ŒhV2p?ˆä"Bûþ£?'ÚÜlùÏ?–}þØ)T¯?ï¿{?n?O=W¡å?¨¶ ÍôG›?«iÏG#À?¿Vƒ®1'v?ÂØl&Ó?ê‰Í}Z‰7?ÃÒÐvAÚ?ƶHÃËr?¤.´
LO"?Êcÿ˜Ý-ï?©œ{ÜO$á?ã¹mèÕòç?­ž'!ÚB?•Üĺzó?‡F¸‡¢‡?»'÷½N¦?°[ä‹#?ëàÀ20Wf?±"öóև4FGL J1705.1-4748?éJ¼‡@À+†±_ˆýÀ9«8bGÀ:ä€üê¡Ê@C"~øX—@+ôË—¦?ÔÏ ´?ØôóT¡@ß	ß3Ø@õkšWÛ?ï{úýŒ³,¿æêÛuÜûï¿äXŸ›fM¿élá8"œ¿åÆ×õõ»¿ïÿÚ
¢ñ1UNASNone?á$˜#?Ãͯ«ÕÉ?À6ÝÆÆ?¼IÀw.í0?ÕÈGìVÅÛ?ÃpJlÝ¥?Æie˜É`?Àº)᪃?©ÚiPÖøR?°¶F/¢•?èÈ'Œ^#?ÁNÒǐU?Êq´ÃVra?¥38W'ZF?Ä´÷°«L?§ôÜáçá4?ä6Tã#x"?­‰
¥¼'Ä?³ipÄCoØ?–Ú¥µ^±?·»ÀÇçÒß?¤r®Ý{õH?ê›YÎz—¨?§¿_zìzC4FGL J1705.2-3850?'þµä™k?õÌ߬£a™À:
E®_ú<À;Ë°Àý‹±@Qlut c?þ(j'TÙ?ÑYF'ÆCq?êøPV×@0šú©]@3D™âê›?îÊâa‰‡Ô¿ÏSJ˜Õy¿ÒZ-òï¡¿ß9çíºƒ¿ïó£¼2?舘TõûšUNASNone?½©ÎÒDxP?³d_I¯½?Áçù<½‡å?»¹œ{‹yS?çÐÇֈü?ÁuåüA¥?¾#ÀÙ]iÐ?Á¨õÄhÁ¿?μ•-á?ËءЏ?äŒb™\?ÍM)%*(k?ÓáœËM?ª"…Ø?ÐÔç"Ur?¬›(ežÖŸ?ÛJF¡]Ž?®‹ð«Á ?Äّ¿ž#¶?©Ð)æ®-¶?Ôg›^_d?¼Q'úñºš?à–BiG`?ºêvû½¨4FGL J1705.4-4850?ïÀ¨M€U?ÀÌ}´'mÀ:9V"tnÀ;‹«‹3¥I@8‰ëPÆl@S|~֟´?ÖœÈù¶?æ‡ÁÕÍÒ@ìMìm@8JŸo?å',Rnaݿ∉ÁµA–¿Ú͈ßb%º¿é¹ëžŸÿ¿ð?ïÿÿÊPËUNASNone?Öä•TáhÝ?ѝQIԜ?¬_ó90?±&/kÔ?âǶ!ýh'?Ðޑã^È?Ò-Êïƒü°?È …¶Ôi`?´‡âD)X\?¹Þ{ˆ†ó{?äX?¸Ö?És¸‹X?ÑCìÅl?°3\ŒAÿž?Íkâr,#{?¯C°`¬Øª?ྕÛ?±¿Eÿdpk?ÓoIGqÃ?³k⛤?´@–øßT?¡·%Žúýž?ãÀH}E´?µ
‰Sûd4FGL J1705.5+2907?ç9Ÿõíò%@AR¤~Ïé¸À:¿5ÜZßJÀ<\m.׃à@ùpâ†@Ðfd¸ç=?Ȓõ%0'?¶V¯d1,ô?èäK8ãv\?þŒ³t·?Ùiå‡ó¿ßsd%Ä`¿êA_f¿ç	OŸz"+¿îìSE!rA¿ïì`Eºõ4UNASNone?ìñ½Ýs?¯ßTüã¢@?'[‹ÞTlé?ŒË,~XV?³à'«ù3?­<>[d"¦?î/ˆx}Ó?¢Ì÷œP]?àYêwÙ?"®îSb:(?¨Áa¨0þ?žd8×[f±?ìÑԌŠu¿?šs/øÜ®?•öÞÒð?"çABüז?³ó¤÷Ð?•¬
i8?ì~ö9Ðۓ?–Òî¶(÷>?¥'šI"?y‡òV\	?±@…dpþÏ?|¶PT4FGL J1706.2-4950?å0[ÆÀžÇ†;îÄÀ:ðp@üÀ;ƒ€ýÁa_@§l®)±@‡ãúû÷?ЯIĚ#W?ÞúôþD>@e‰ýDcÝ?ø
t";¿¿å\·ûeg¿ÖóI¨Pí¿ã¾V<"¿ëä ©m¿î÷Æ`!'î?ÞFžJ''UNASNone?˜,‰=?•9AåV?š³"zÔã?œ†èÁs+?îi·"ð‡?¤_æфˆ3?È^pÅOq)?ÄU'Ï\sˆ?¼ñQÃ?¾åŠŒø4?æVü­ù}?Æ¥R*÷Úq?ÅM痰ß?¡—µÑ1Ép?ÄH€çN?¡ËF¨£z?匳ùÙä,?©ék²º[?Ã+-¯?£å,'0Ú?È×Æ0Òÿ?«Âä/MìE?åírŸy?°i¹Ðîè4FGL J1706.4-4609¿àÂk»oáÀ	ÄȼœÓáÀ9¬¡´NÀ:ÜC8cõ@ !¾‡z]@åàdYEì?ÜnÖwpyæ?ÖÝqà˜Æ?ýƒ3ü†Ï?þ±ì<É¿ïô‡'YY8?ïú:þпׅì~à¿äW¬ŸZή¿ê¥cÒ7oÙ¿ÕW`NjUNASNone?ºPvóU?°Ö[å¡?ÈhFµÉ6?Á@A'çç?æ›ë¯R?ÃÁ`OUZÜ?¼^
k.ë?¶4þ•?°•'{Œý‡?²"SD;=è?êaŒƒ('í?¼Q©i¡®?ÀñZ£TÍ|?œ*ʗê?ǵñ½]¹?¨Àak(Ê?åÖ,çÆõ3?«™þà©?´rÏs´+?—À«'~ì?²}_-»ø
?¦½*ÒMØ2?ë!ú+è*y?ª±Ztõ¡ÿ4FGL J1706.4-4649c¿'›ãý"5šÀüœü$©-À9Ëû¹IÀ:ôÞW(Ü@=GöŽ½@^ú|2€†?Ö÷Ö»¸þ9?íý«w@	ízÂ=ý'?ÿ¦Tè凿ïÿ¿h`;ª?ïý­àx{<¿éðˆ=ќÀ¿ìZ¬‰`fr¿ì…;=ð?ÊÊ¢{žHUNASNone1?¿t¢èœªs?»s¼¯Tl{?³Jøw?³¼]Ý¡öH?顈y©‹¤?Ây®ü
Ì?¼`
­Ìq?¾¥õT¦öÍ?Ë	\?:t§?ÈKí=uŒ?å»<î{©H?Ɏv`\¸%?Æôâu$ÚX?§ŸöDE?Ŕ@»É#?¥î=ô®ç?äÝ·\×!?¯´QïöF? "Q)½?‹f8Îw6‡?Ý=t³´?½ÎÖ4Ü?àX@³-ŠV?½h¦E44FGL J1706.5-4023c?잏8ÜYL?͒Fiö¦À8…™1"ÎÀ:g°éAx@Xô"&@qœûMê?Ɂ©ù8:¯?ďHy]d@o¿@OÂ@*5³–?ïýFA­¿È+³1fª¿æÅ»Áã¿è(žŸ'×Þ¿ë\½جտïÿúÁҝÇUNASNone8?Ô×®"×Øî?×ê¸{ê'î?•~¹Âfö? HçÑ}N?äè2íŽR?×TJgÉQÆ?­¤3Ñíͤ?ªØ{<7"1?§/+ð‰??­ïê¡!–1?ì²Ê؏,?µ<<(Ɖx?ÉWÐks,b?ª;gZ°'è?¼¨°Éi'?¢w×Ñ8({?æõËöV?¬÷,è\4T?£wˆYÐ?j	Êz<? Â¾A&x°?Š×gìF1?íÂ|£gûu?•:Ëí ÂÄ4FGL J1706.7-5525?â±d0×
mÀ!"½8SLÀ:-únƇÀ;¯2c)›@ÿwšôŽ@°\‰mÒk?îŽ|?@²£?àµë÷öF@î¯?ôÖ@^Ѭ°w­?éՌŸ
FÖ¿äÜ¥R4€:¿ëM£Œa¢²¿è!ìÿ.¥¿ÛBwî¨j¿Öº
›5¦UNASNone?Õ"©¿"ɲ?ļVwü•e?Ô<áÌBJK?ÉÈíOªŸÌ?Ö tt(ì?È.Óo¤¬F?ÝmR­Ç?жüVËÒ?®:ó½cì?µzk;V¾d?ß)…Þ{?Îàˆ¡[Ëó?ÛÁñoã‰ü?®
u	WÝê?Ã"ô}9øo?¦‹§ðû™?Ú¬"QyÍ?¬<&¦V»c?åv¬1±ö?Âæq?"ð€X ?¢H2š±?Óӟ˜h›²?ÁíW×öÙ4FGL J1706.8-4540¿ê¤B€ÆÀðîÐ,ӞÀ9
:¥"À:x3⅛¶@Òå°@Äú¦#ë˜?Êꡞ÷?ÍWåÐD&@q£EêÅÜ@5,ìG;~?>t3¿è 'w"Œ¿è<yÎ"7b¿ëZÉD'¿äÃ4½ÌÔ¯¿è
q=Yý¢UNASNone?ÒϞ3¸q?̉ƒÂ?Å0@>â?ÆÔw1å	Ï?áT)í?Êﺨ_0î?Àãt—½\í?»ttzâ°?¤ÑI™muô?©_S_ˆé?êz@yÑe?½E›ÿŒ\?Èo<ÄNº?§SKÚï*?À|µÔL?¤=6²¹
P?åÄëPÙê¾?¬gµ
cØÔ?¬²g/hú?"6ÈAèÀ?©@|õ WÅ?—½'K@½ƒ?í~'l;?š\ž^½3¬4FGL J1706.8+1319¿á®wEB«@=
ù½Æ À::¼µ'•À;ó
÷9ˆ@tŠ‡¿@˒}E¥ü?ÁnÝÃÀÄ?³jzF?À»~ãH@EÝ
$q¿ä#gC8N¿ä>Yl'à¿ì›Cót×B¿èÈΪŸ¿êb!LÖÈ¿ïðCÊZ+ÆUNASNone?ïFU	I<´?"¯È:mÆ?~"‡I;?y–r"NË?hsjR9?À®¶ö8(?ïJ.—€x"?"þóÌO*<?^fMw:æü?kÙOm†«?"ÓÈ8}MU?'˸
ˉ?ëLë¶
,\?§Â5a`õ/?ü"B?CGMPV?¾™Îþ?£›Õ½¦b?îä&Ô;€®?‡n&*zá?yâŠ,…7?jh¤û۔A?'ñÈö?…gß.gj	4FGL J1707.6-5351¿å<–¨ðÆôÀßþmXÈïÀ:dT§!A™À;ÁåN£Ò@—›±vÚþ@œ zûI?ƀ"9»¸}?ŠéÖë+)?ÈæX%?èhkêòÃ?ï´Ó³¬j¿ãSæ1!àû¿ê.‹-Æ¿ä㮀†x*¿àÒ1@ìF¿Ü¥Ûüëx‰UNASNone?Ú\;gE?Çj¥J)?†£ ·y~1?'ÒV{¨O?âwUöîå?Ǖ·fIT"?Óx+*Ϟ?Èø¼¶eF<?XMssô‰?™='FÎ9?åΉ4Êa*?ÈòÕÐýV?âJ%S©îã?°àQÙAÙ?£{+"šË?‡üÏ=Ÿ™?ØüOèÈÕ?°…o`ؐ?Õlÿ¢"Ü?®ñ˞ö?©öO?•-3¦»ù?ãìïoQ"?¯°pöV@p4FGL J1708.2+5519¿²ˆãÙå¬E@BE"V!uÀ:ò¼~ ïÏÀ<‰
ä¹S@4,AQ"@ÁÛsX½?Á~$É
$¬¿²¿^z3͸?ðÞu†"Ú@•^XûIJ?ìñeh9¥=¿êŽÆÚ
M¿éóëÇkd¿â³@S'D¿ïÿï¤h)µ?ïÿyYˆUNASNone?ï¯g°Ð8?'¿…(ï²?€™lF.Õ?Ðɞ¥?\e<-†çé?_IÕ¥	kÍ?üôš?£ÄÇ6j?teY­ß ?†ƒl Vî¯?£t¡Äúúu?¡ô¥à?íÞ·¥ŠüØ?'¸i‡¯º'?‡ŽìvSÒs?wù?fW?¬0ʉ»=Ú?îcÄqà(?ï+ûZ—Ø?"à&ƒ¤)?€9´£×rè?s/Ê4¢?'cº[3‹?T%>»Ø4FGL J1708.8-0923?ë0rÛâ@1Îû"‰µÀ9éÓbCÏÀ;tgVPn­@¨¯Ýþ£_@Æç£è`?ÏêéWòÛ)?ÎÀ|œÞ…@úälü'?ý¢™gŌ?ï;š«'"?ë†'_8u¿æ3ý}Ħä¿è:¥Ž¦¿ïü‰Þ™–¿ïÿþBe«+UNASNone3FGL J1709.4-0917?éú*kÀ^Õ?¼ý"þp_
?¬…SI¶õ%?¯FiŠÞʌ?Àö~Çd?·y:é†?àÂø~ڒ%?ÊoÓ¢cE?Ó,"̽ò¶?Êuñç?ƛkÒ?ºÒ<ùGÅv?Ü4IŒ2W?±!èâØ<?'›†
z?£"…°3>?ڊh°Ì£±?®—…•HJq?ÓÑìÏf?®ò¿ÙàÖ?П²•Œ?¶(?ר0?ÜDÉ`›
?´pO3àÖ.4FGL J1709.4-2127¿ÇZ\Þ¹o‰@%ãU>S"À;8ÿI÷š×À<ǂ4"F|@ ÝɅ¯Ô?ûT^[Õé¬?׆ncàÐ?ïò%ÀoF@ُ>Õ(?üïTa+>¿ï2QÁ"³§?ïýµ7"Ñ‹¿Ørê"ž ?Úu^<¿íAWîÔ^'¿ïýÜÚa
UNASNone?àÝ0Þɟœ?ÆHɑ:?ӝõ}´e?Ãúð<<'*?ÅOQŠÊÆ?¾r@SÙ%?ÄçTv£0?Ét¹ðh8?æN,éxÇ?м‡*Iî%?ÂÄh?ãy°?Â@/àiJ?Ý xüüé?¶Ÿ¡ŽiÈC?Ö4.¿?¶ƒsôôz?ɍÍ|¯?«x%£þ6ø?ÈâƒMÞ<?¿ÁÓy`'?å+ÅÅ`-?È©mE"o?Âneœ¡3?¹•Á4FGL J1709.4-0328?ļ\Û±}@4ÅE¥ü~kÀ9hAK#êÁÀ;µ´+W€@˜XpÚ^@ORƒZ'ô?ºÛÅc!?¼…ùԗÇ\@tt–ªÑÐ@ÌûÎÂñ,?ïʑô‰ª8¿æÃ:aû›¿ä	z!Úh¿æFÔ©¿êIßÇü.¿ïÿ (ÿӊUNASNone3FGL J1709.5-0335?êÃOÅ?³êÈ¬?¥õ™v»n²?œyQß²4ø?¾ì`Ȕ H?²4Âá¶d?èm™ Œ¸?À¾+'ä"€?½Q¦»•<Ï?º¬õž¼fŸ?¿A"f]q?±YÔîñR?ç]«z
…?¬îÍG(8U?³Fõ_Ë?œÂs5??ÊC'gä[?§…ëµ±©s?ã`nNÈà
?¥¿VëQ¶?Âxek"±Û?ŸpÇYFóh?Ðð¬Üæþ?¢X¬)³Š4FGL J1709.9-0900?ïíiÑfÖ@1ÆüvÀ9þCiâÀ;­iQ;@z*¨J6…@Æpº}>ð?Êpkø̄þ?âžÏ™/çN@œ4;pïV@ìÞDïHM?ïö8 WäC¿â @|ÇÑ»¿âºJÿ'¬˜¿éUao0º¿î×nF.¸z¿ïÿýç!éUNASNone?ß½éö]<‹?ÇͬJû?ÚÔpæq%?ÈÚ÷̏E±?·	bñIC?±Ðš½ e?ÆîKªô#?Æe§Ààº?åš"† þq?ͪä?©*=e?½xê†9¥£?Ð,€ýQýo?¬I:ô¸`?Úž̰Ì<?±øf*Í ?Õ
À5ý6U?°9wxïìy?³'¿#Àö?"^ 5‡Ð?âëÖ¦Ò¬?´ûAàG£Û?ÕeHÃûji?³à=ª-ŠÚ4FGL J1710.0+4629¿ïínýR•h@B/Øf€À;	|gY«mÀ<¿¹üæp@±Æáü4?ü=''N#z?׬9¯N?ÚÚÙjj&@?mƒ'˜?÷Ï'EZ?¿C¬ÁÙB–¿è¸V¿×-۝ôr¿Ý"§BÔ¿èY`Y+"¿ïø"PŒàNUNASNone3FGL J1709.9+4624?î&xç"£ò?¥&ËÌÑþg?‰Gˆ3ÊJ?ŠAKï;?§F€ã;
?£^ê߯j?éÙ¦­q\?¾Èµ%ÍsW?³_æTU ?µf&h;?½×|Æ@~?±>0˜÷÷?ë–U"š4?£O=H³N?¡0
­ÊåJ?\‡l@‡?ºµKu»º?Ÿ31±3X?ãosr‰j?¯"€NØË?´\]á»ö?¤dr÷?Ó®Á¢~.?­3"|G?4FGL J1710.1-4541¿îöÏsù«À·'Ôà˜À9Òí˜oWÀ:Ä]ºÆ:@ ÝÒÕzp_@­D¦">?ÅáÈÇÚt«¿öå=öŸ?ß$¥Ñ¶A?ûǕ*t¿èI ]?é|×V"ŠŒ¿µIÖã§å¿é=êFZWd¿å<jIIõí¿Û+Í
dl'UNASNone?¬¹o?
¾¯?³˜šÓs¹?†_GRD?•{¼
?íÚìÌ6Ì?¶ªÚKËa?Éó³\A"?ÀÑGZG?à?"‡ùOá?'ÙE–Y˜£?émc-ìÀ?ÀÑqƒÛÀ?ƽþ–©?¤ž$ƒG*¨?²{³[
.?—ÓÌ9Zj?è	ï¶?¦ß¢ÉO‰"?µÏaëO°R? Ã™Æ+]?Š²¡´ç/·?ƒ<šºwö?ìÛI;Âm7?¢
û$Üû4FGL J1710.3-3039¿èÛ£•NŽâ@¯¸á]}ŠÀ9íŒa¢²GÀ;"\sž]N@Ž`¹~;o@Ž8¿,Ñ?Î=ÄfKä?Õ]mÄS¬z@˜:ôȔ@0…·e¿·òÅYç?å«ö"o³í?…§	Þiñû¿á¸FB"‰è¿é¶É™"{¿ïò…Ãù¿tUNASNone?µÖ,´å?'Fäå—)?¬/ãã¿?©š¼"Š'?íOb\?­.lt<ð¯?Ã]Bqˆ?¶§~Þ¡eP?Æ$ßþž?À1U©Ósz?壦+¹´·?Á†Ì\œÊ·?˨œ|²c?¦·¨ƒXM?Æ=cwhø£?¥¾ÞÎao?ㆃ;•=?®eœÕÝx?ÌäZ¦D{?¥J€íDÿ?Ã8•±`$…?§› "°3?ãøÄþe¿?®`\ÇŠû4FGL J1710.8+1135?åý(8·	@;‡dº"¼À:²?d™ÝŒÀ<*.wÐ@p›ž‹@}ãZ­Ë?Ù´…-Pñ?ïÿþˆ0»Š@¾¼@ŽÉ@ÇÀv?ïíöé	:¿Üè@Ü;Ç¿îÓä¿ïÿÀ¿ù)Í?ïûJî:Ü¿ïþ@ý÷DUNASNone?ïe­ê–ç?Fë†ñ6?Žáº]Àð†?šDaúYBM?nÌ	žeUÔ?€þe8ÔÕ?ëÔr-©?ÅÚƍ‰?³"®·	à?À}‹6?´F­·|­ø?²%Á?é3ڀ[¨Û?¨W'ø@#?³¥k¥ã³á?ì"ì/?Á]à+Ÿ'¡?¡êàϕ§1?ìŠ]Jcî?´á°6¹þ?˜/­®_¶?¤þ›ÖÔ£â?µ¬‹:AH¤?°v4føqå4FGL J1711.0-3002¿ïÜٕ©@'Õü3ÃÀ9ç…w£¥ŒÀ<ìxc¾ì@äQ&@áf?È9ÜÛÖ}?ï@r¶ÖÁ@Å?9ѳ?ðSœà ?ïÿÿ)@k*¿â pÎI¿Ñœž|ƒ8¿êYÇòrxÿïü"Åý¥³¿ïÛÖ¿•UNASNone?¡˜¹"=d[?µû)zY'Ÿ?æ `q:"ô?̑Ô.—n5?ь'ùD
?ÊÇý"Á?‡Œ,7'?Ž(½Å){?é;·âpT?ÊìG·:ÜÙ?ɟ7³{=?ÉÐjaŒì?µVҖ—j¬?™)l#Ø:?åhNÀê?°6Ðé8?ϳ[´±<?¬X;Øä?/¶‹Ò¹2?"Ÿƒ†ˆ²y?îÂL~	K?—Ãú1\?£»"œ¤?–õ''ïÂR4FGL J1711.4-2526?ꢖ.oË@ ‹ææS†À9¾çBsBÀ;€¨AÓ	'@ž†¦!è2@©õ1?ȇiÁ9Æ ?Ìmš7NJç@MNûÖ7@ºJyJï'?ïì2ðî¿é¨/"BAÄ¿ã%DȆìï¿çÝî'ð2-¿ïÿ÷fÔJp?ïÿ!ž5_³UNASNone?ÓW?WìªA?ÁýÛËîi2?™VÕyޅi?"ÁÑÍ3¦è?剩¨:¶´?ÂltCBà"?à+të¯ô,?Íåâ\ÇñÁ?­Â½Z…®`?±¬ù®nO?Ûð¾}OaÜ?Ì¿YŽê˜?ÜEÎJ\?®PúQߒ‹?»»Mo¼¹?žö×És"?ÜþæÕÆ´_?¬±Nuæ}?â‹ïðû?µ«3à÷å…?©~Çc+ç?"3é'Ûÿ?׸Hà1¤V?µ@r^êò@4FGL J1711.9-1922¿èsf*Æ@'PoiDg8À:]^ˆK"|À<eˆEßÞ@g¥3€µó?þÆxõ?Æ6Ükü(?à{:Ôd¬@Ê~=ó?ütá0‡o?îß»‡*+M?î!ÆßM¿Ç?œ7®˜¿à}€(¯K³¿ìÁ=ÐE'¿ïÿßHÐSjUNASNone?°˜š!*í?¥ÂFÛrC†?ê€Ù"š8??ºÎ$_¡	?»`œÊPç?´òõaJÁï?¬AX´'Mi?®È9Òï?éÖzĄ	ñ?ÂE¨ô^ž?Á•¾ÀÏDâ?¾zðVJ3?»á:Ÿµ=Ó?£DKT†"<?çÛ>%ÅÒ`?¯('
@4?¢j–?£Nã?»"?{O	ý? ²$É£-?棠D¾?´stü7¶H?Çà]ÍHL?®χ.3‹4FGL J1712.9-4105?ê8Oä]¦é¿ò—7¿‰î+À:NM6êwØÀ;qäõ8@#Áåh$,?ý"B
y?Æȶè‰ì¨¿+L€ûµ?½YVˆwÞ3@cho«­?Ô´­Vœ¿ïùͶט?ïùÞHS'?³LyKµ¿ï€Ê`"?ê"ÄÀŽÐéUNASNone?ÑEg©Þ³?Åì–Ë|æí?nV–ód?q§qwpЖ?ç>õ"ý³?Åýüi­^?ÓÎFªœ?Ïo}rÝvè?uÝ*-¾Ç?"H¿–Æø?æKÞ¬ Ï4?ÏCsõ–v@?×Ìa:³mq?°ÒâËF*¦?¯¿¬Íb!?–ÇÆ>ƒ?âÔ¡és%?°&;H=9?ۚoÞ3ž?¾5бÖúE?‰×3Úþ?4>ÝÖ³?áËkA~b¸?¾\BR4FGL J1713.0-0521¿ìB@ƒeŒ@3	Ò9XÀ9±ZI!²À;Š$_ZÙj@_µ֟	@/«|,Ò?ˋ"ˆk?Ҝ"$'\@ob@ÛBà™Þ¿ßÞßHûG¿å¾»öº²¿ëò¢IkƒÝ¿åÈ7½±¿ïóˆ'	?íðh]a…UNASNone?î)íøExš?¦ÌÁhà¦?™•R{M'?›ƒ˯¿? –œÒjÏÜ? !{é[Š?ë«Â½°åE?¿"Z¥3ûº?¬y'ñè‰?´ø"ÐK–?´e!ëaš?°ééHË@Å?åg8~å£0?°ª'"àH?µRqzñ³?œ¨f›'m)?ÏÛtË«úd?¬	ü™N?é˜ÔÑ_Ò¿?¯û1Á0o?ž´&çüæÛ?Š^A"HÔ?ÅÆ'݁'?­úãÒý=@4FGL J1713.0-4236c?êxßÚh
RÀˆãƒÈvýÀ9t«ášº+À:Î	ԕ+@ Q(;³_@såÍNÓ?ÏÔ߀Xªç?Ïo¹vXÌË@ía¥6…Î?ýZ
…#ÀÏ?ï:`Nq¿ávŸLa¿ÜI@¢B¶¿ãy[k`¡+¿éÊìW¬@¿ïóGŠÙvUNASNone ?¼¸(ìiÔ?¯T¼nàuL?»Å@ڟ?³Â4d,J?éýb:Wq?ºù£ý^xC?¸Ô3{vù7?´&®7až?©¿nÙñŸJ?«ü¬ªCò:?ëI'¢òä?·~ÈJ±ä'?ÅD†^LIE?£`çÀ™´?¿õooû™‰? ˜Æ›y?æ°0zmz}?¨+	oyº•?¢'ØO­ ˜?…åօ»¬Í?¸Àsø»Á?¢lðla•Ó?ë¿Ä¦~?£CÍmeŠã4FGL J1714.6+3228?à[ídz†Œ@@ÆÂT£ÆÀ;ª{jÚinÀ<äŽ^Òô.@!õè?û³5L'?Ñõ£KÛ¡?²º·¡lvÌ?ã'3¡m"˜@O?w9Gt¿ï îzÔ]?ïò®Þ¥<e¿Õ'*g2¿ïá.žxük?ï–kFŸ÷'¿Ü¾ïÿ×¼UNASNone?ïãÁ¤Ãn?n¹×n‰i:?$'Ëmc?%gh²Yh?jýh¿ÛK?n5›tÿxÉ?ï4¬RXr°?«…î…Z?XGæzé?wý¶dl?—ê%sBH?ªÉS±xEã?í`5á—h?–J›=9Ê?'-§ñ{ò?~œÎ
°|n?±?IRÒu;?" Õ¾wgæ?ïƒ4}5¥p?…Àßê?"…¯ƒ¨, ?1]¬Z2gÝ?ŽèÉôˆ‡?…¼·1:)4FGL J1714.8-1421¿ã_û>éäz@+·+ˆDÀÀ:™âàíÀ<Fƒ
â@Rzé*?úË$£Mx?׈†KÞû£?áÂZ£Š´@E܃#6@AmÙ!næ¿ï""Ÿ´»´?ïýuÁÎ#¿ÚñÞ"Š™¿ÕÝÏßäØ¿ås‡ìÈ뗿ïý
a½_GUNASNone?ê¦7»¡lÉ?¸.½â!?¤š+7JZK?œÝÎÄÿeQ?À@–C§¶H?µÐÙêÆ\?êÚ e'_Z?»­o&#96?¤¹–4dq??§¨PÀ û·?¾Ò1¹:̏?·]?c2ÂÃ?æñȎ$²?¯ñrRT?³fÙ^í€?š×Ũ˜è+?Ê®*ZÀ"y?ª¬a‰!;9?ãêe‡^£é?°¼€•\ü?¤^±:"?"5Z^;ãS?՟^Ðÿ0Û?±œÇÍXhc4FGL J1714.8-3849¿ì"üÛ¢…¿ÀéÕÖX½À8@NÕP)
À9Ì:䜸@—áŸ@2êRï'?Áùh6J>è?͉—Bý*¹@Û%ö3Îd?úX»¾¶S?ï¯Ö燿åÌÞý';¿àKeè'%¿åìŒñª²¿ìV/n¿ìêßBEJUNASNone?€A¦ZÆj¹?wÓ¿þ–Ûv?ȇK_	¯–?Âõ5NJP?é&ŽÒzq?Â>9u'¨?Ž·){ëh?•Xµ¯¨
?¹Ä5r
Rb?·5P˜a?ìOvuÆ?·¢d¥
?¬b9Æ×L?'\wåwÀ?Ð¸1Ñ?°1Ûª
:<?æ3€UÙ£?°XK*Mܧ?M‡BÌß.W??æÜÇo¿v?´Œ%Ðå)"?ž‹gê"í3?ígu0#?ž£Hüt?‰4FGL J1714.9-3324?ævq€ÇÞ@ö¥
k#À9oNäHÀ;*¯ÿ6¬d@ÅÛêÌçû@òzÞÃo?Țk%½Ô·?Û}¶Äͤä@5" ¼8?óH}ˆkI?ÚZÀÀÏéb¿ßð½Âôu¿ÜZе
¿ä3ò«ƒ¦é¿ìl¸?wT¿ïþ'¼ÞB@UNASNone3FGL J1714.6-3327?"¹šR]5?z!ŒŒ¡N5?Îãa«`‰\?Î}—?çôA,Δ4?è"7†î	?¡)Däø0J?­àxJvÃ?Úy¨sJ…%?ÎíšÏåà?ᰗx:i?ÎP¦<~%H?³Ótô£çz?'"ü"o0*?Ùº¯ÇÍ?´ïCdïç?à¨9×^Ÿ+?´&Xò×\?'èþ\ûdÈ?x7ª³Qj?Ðwp¬9
i?±Ì¨
³s?ç,ÿ¶ûž%?²L'¹iÍþ4FGL J1715.7-4239?î_ð;ÍóÀðCRe(À9ì) ã9÷À;­e(xÅ@¸dC¡j@õÆÛò¾?ЂV¼¥7]?°	ž¡l2?èk¤Éx"v@ٍ\õNv¿Ûàÿß"?ï¸x·¡Â]¿è3¤Ýšzj¿ëU—Ià?yë‰%ƒU¿ïÍõ´L£UNASNone?ÐÃCu³ ?È!!~‹?Œ¹*·°
þ?Bå,»s?ç+yšGµ"?Ã莝þA?Úßd{{ŸD?ÊNað,3?rr¼0-?ˆþƍ›Š?âkhJ<+þ?Éþ®-ˆW?σµ^$sv?©¬éåÜOÜ?µÜôüc»Þ?œÝÐÚS?åctêk¨?«ŽÒH¨–{?â ‹™u?¸A'Ôšå¥?uã"ßEjÐ?r÷ÑÖúÿ?ÛhnÖa·j?¸7"»"/4FGL J1716.1+2309?ÞÊ8/=Җ@>§T~–À:}ÜygËÀ<~¾b¦¾@ 4‹Âktî?ü‹vUDz²?Ä1}{€Õ?ÂFÒâ»vŽ@F}ÄY?ú<–÷RÝH¿ïiaB?ïÿîbHÊt¿àVà¡ë͙¿Ég]äâî¿é
Ä^ê<¿Çâðµ	UNASNone?ï
²êç$?"3û
y2ã?}bHY	€Ñ?|Ô-±¾žÝ?–õWŒ`»W?'dúEˆM?î&ƒ'?«>­…ÜF?BAa|ãq?†Å+ßã‹?¦Œ}×ä?¡mæp1?íÜ££?•dIùÿ'?Œþ"Õµ?'‡ë«.?°{0œM?'LG:`?êß~RkÙ? ùG`:ô?±Óс¥© ?˜ÓߞWé?·0=›Æ÷š?•5üFc-í4FGL J1716.1-4342c?Ù<£›oÜÀ	U°5½Q/À9§>ïÿ×¼À:îfWLíï@~Êö†@¿–áXu?ÒéWG²J?ٗ֠áž@
/Â=&Ñü@-ø¦š^?ï
užèó¿æ"_@Ø7¿ä˜=Î펿ëÉZQ…-Ò¿äس|
¿ïÿäÅøUNASNone)?ºªe–`?®\ƒ O«j?¯œ­'ÅÖø?§'Råڒ?ê°ñú0Òd?µu"'À?úŒцP?¼áÐþHs?¥¬)ø·Ê?©£Ûœ?鶚[€!Ë?¾Ft­'ú?ƙ#ÙÖR?£ñ"tNö?¯]Öð'?¢uñÉàJ_?åÓaÎb?ªÎnÏp?²P®»Ô'A?"öË·ZÙP?ªÁœ7ÅH?"Ñ|ÚõN¶?ì	Ñ.ÁþÄ?žfÛLP'Ò4FGL J1716.9-4152?íAIò<sÀÖÆÞvB|À9½laR*oÀ;"÷í@'qÓW@7"¹hkú?ÍWÙu&É?ʧ"Är¶+@j <¶i´?û†2(œ+?ï5¹pޏ?ïg,_›–¿ØÝZ»g¿äE‹àsr¾¿èªÜb§¿ïþîB=g?UNASNone?Æ2–öa?¼²ýåoÛ)?§îj3ª˜?£ýŒì¶U?èôsŸFœ÷?¾¤]èëmä?Ákæ^ŸxÅ?·ëpʦ0=?¦"TsÛ¼–?­-À˨ì?ê;Ñ!f?»ùbßN?˺Mžm)?§éhEQ?¸Úà¢?˜ÕÞ豀,?åö*Pu?ªCx7?ÄNi:=µ4?¦œ'`Fã?À°ë3ÓÑ?©pÓby!Á?æÀ_v£¾?±|ÑÓÞ`õ4FGL J1717.0-3218¿×Z‰»w‡B@
WýO0ÀÀ9älòq¢À;6q'Šˆ…@ íãLì@¡ÞËÒÒ?Ã*[sCD¿C10ǾZ?¡ñ,}ŒrÀ@Õ®zÒ.6¿ã'㍲b?ïœ)@ìt¿å,"½ð¿èó`_fAþ¿èkÆ¢'9ú?¸ˆ_	¥Æ#UNASNone?à¢êà‰Ù?È¢0ò.?–¸ªî?‹˜kèa|]?ÝÏL$y"Ý?È~>" ?â^!h1?ÈÖf<Izé?ƒú""-ã…?–…½T]?Û"/#À?Èj½"éH¶?؂WRŽ?±ú¯°ªCa?®Dý`'Í?"<@Xáfx?áڄ}ÂôÃ?± +®?âYþiÛø.?±F=Ũ»?ŽVx—k"(?ŠÄààx?ÚYOgŒ³?±R†¨Ê4FGL J1717.5-5804?ígšlíÀ'hRÀ:kàèãƒÈÀ<~Êx_@G2?˜F]?üX#ã4_?ÊÚ*BôœJ?èð¾C
Â@5I¢
c@¥®¥ÅL?ìMIÊNmK¿â¡Ý_ìû¿•ˆÞWÜ¿à8IÝï‰æ¿ïÆd""T‹¿ïý	«zl®UNASNone3FGL J1717.6-5802?º÷æq
2?·'ë®è¤?êG1?À{Å¢ 4þ?µ¸?wUm‹?µvì<à?ª8fÃþ#?­mï®l?åçŒøå¹?É萍g?ÐéÙ5¼	?ȝ¿€‡?¿%}ÍÄ©á?£E4.
%A?çcvg'÷?¯VàÌVI?ÄS³?3?¥<Oó_ß?Â…"
Ç?¥èÐÃsm?äaڢΦ?·Uõpž0?Ìj~?ẟ?°hï_ð4FGL J1717.5-4022¿ÁnÈ=Nž¿÷SŒdý±À:–Í[h£À<Br©jÈ@ B–áÙNe?ÿƒ\=¹?Õ2køvžÃ?ïùƒ^ıu@á¹Þ³?ý:˜‡ É¿ärâ?û˜'¿ïÿä†ýµ£?ïþú·Šñ¿Ø‹*k
•¿ì°¡óÛ/¿ïé˜_‡ÏîUNASNone?°/ýCÔá-?°ÕÌèљ?Äñفü·?¼ë,8Ê®?èóÃá$ä¬?Á\'I&â6?¬ÞBKßÍ?±Ðå²AÞû?ƌýk¬ß?Ç{*ü$?èŽàð
>?Çžuý"ô?ÐãO}×ì?°ÞôQ¾÷?Û
…mww+?µÌNPjQ?Ô+
°ç?­RžÛ}?¶¢K+"Ï£?¥¢˜Hٜ?ßùvè'¢?ÆO×ט´?Ú]öL˜ÿu?ÃªŒP4FGL J1717.6-4404?ÏÙk@ÀºpÀ¿¸fä;À9"šv8kÀ:Ûµ#bۗ@f_>ÿÅ@8Z\lèa?ÒI䥆?ÕޏÂÖ(ì@Dy¬"H@n"³*å?ïüPþ .‰¿íQ9®ww0¿ÞJªž#Áü¿è¬Fàˆ¿ë•¢ß='³¿ïúÂÇ;=UNASNone3FGL J1717.6-4404?Ė]ñÂ%J?¹‡Û~žÿ?±zÅí¹Gc?Á§"24?è«ÅØMÁ?Ãì‡ñ¶ˆ?ÆuɘÑ)¶?½´L_§†? 2+È?£Üõ_übÀ?é_jÝ<½'?¾ªóYi8Þ?Ëî¼äFÔ?¨—ÈÛÍÈd?Ádk䄶—? 4NÙ'?ä«6¥À¦?«&ú€v	?´¤äËÛe?•3>\ËC?¦øÃ{Y‹?'»šÓé'ô?ìŸ+¶Nû?œ6‰'Ò¹4FGL J1717.8+1955¿å3]oÐP@=1	¾ºÀ:Ë:CȬ­À<bw‰¤Y@Ú Gs1@éºÿDï?¼Ö_Æ?"žgšÕ*?À†D}2…¹@¯Sj5S?CtÉÖ¿°Å'<3¿êþ'âÆ3V¿èdµVŽ'¿«d]D 7пè™ÇâWMšUNASNone?î4-_uBÑ?¢Ð±©Y_Û?ƒµÑkî£?€ú^3©N?§Ïµ­°*.?¡!"úvŒ?ï*«ÙvÒ?•
ùcâú?_æeHeuõ?o!t%¥á?˜¬|¶Îy?'ôüïÈÙ?ìÖYÑیu?™)ˆ¦[k(?'ƾ຅?'(ŽN_?´Û¸õ²?"Õ¦ÙðNS?îÉn0­"£?‡Ö:Øô5	?oh{†N7?g‹è.L?¡pFmupô?†l¶£´¹4FGL J1717.8+3925?ßfïç¶@A†
¢À;Uî:ތÀ<ɓnÝ-m@ ïñ2@º­,**?ӟ¡[¢?Û>.cëŒÖ@û$ p¸Ð@¶ÁȌ̿ïýíÁ?￧¬_o¿Äó¡ã?*¿åB˜Ì@)¿çï…^y2¿ï¾­àMˆUNASNone?eM?¢Ö¶Æ«?ŒÄ·	ß?†0E-øÏ?¨U'+ì×ü?¡FMµ	÷N?îA»Ü6E¿?¤˜ʅE†?"ÃY™US?Š§£ÙÁL?¦³kúuN¯? ^íy‰•?ëxFz\?¤?"®¸‰?ªUpƒ´?•MœÀõ?ºT‹ü©;?œäžAµVÊ?ìÐÒ2lÒg?˜Î	ÿý¯ ?¤‡AÒ,GZ?È?û'Xy?®k›'=?"þ;i&ç4FGL J1718.6-5821?êöÿ¨rÀ'ø@À:
ùûAÀ;ǁ]b±¦@Õ0‹yp@}G8£µ|?ÁÙ¿¤p7K?´hÊCÛw
?ðŸ-݈ܳ@•»ô7tá?ïÆTdÜ#¿ãªÛuÜûï¿æî!7¿äNMÃiÍ¿îÐüqÖ1¿ïîDنUNASNone?êçB-yûâ?»—VIšÁ?"À&NPèì?Œá5)Bxh?ÁÊò€MóZ?º¨æIЅ(?çƶå^?É'ï±-?‡ÛÖ8ÉØ?Ê:³UB?Ïgg_ø?ÈÀÚT
%ä?æã4»Å?± 7gƒ?­tÏ*¨Ô7?•	\ÞW7§?ÍùHõKá?®Â"ßeÛ
?èE‡ÙQè?¤®Ê
Wß?¬¦áY'?'5±–ù}º?ÇÀX£<áû?¢Y¶jt;4FGL J1719.0-4038¿²níJ
¿ýeÙ($â8À:|Í°ø[À;JuòËd@ µY€.@aøDIÜ?ÇÚDºõŠ?¦C®Öl³²?å>ÖÕdK?üAòMå¼?ï­o¤Ó‰¿çN>f˜¿å<â¿'r¶¿å]'«ŽŽ¤¿á£Ž_©³Ã¿ß1ßá|‡:UNASNone?³Žu™µ×?¤ðnǺ3?`¸V‰'?\g瘠ë?í~¿"r¼?¥/ã0‰EC?Ç@!²æÐX?½ñ_§¯?:§lX" ?ƒÄaƒÜO?éëõ"ë_?½×¼¤)PÎ?ÒqeØX?¬ØYåÈAh?¦«aÎ4?j?"f÷{ÝL*?å\½ÓiÏÝ?¬

ÂA:?Ä•iml?¢ý2aÝ?'9òà´?'ö¢n‰Áã?êiK%£ø?£ô!J‰)4FGL J1719.0-4221?ï
äAôyÀ v}4ßÀ9Á•XÂ8õÀ;A	pÂ
@>nfë@C{Ó?Î!4x®?܉+bYfy@LeáÜ(Š?ök¥¥–}?ïmq½²}–¿x:ì1ŽdÕ¿åYxâií¿è— Ÿ²¸¿ëɉDH"¿ïó<7¾³/UNASNone?­áQ¾8W?¢—æñY?ÅÎpp*³)?½`R«Fdß?è®NÓio°?À(Ä]}?°¶åM¾ÃG?¯ëª¸'†æ?Ê*™¡Kt?Ņ"Cª‹?çi¯ßÔº?Åj£ÛÎ8?¿dlôU"?™ÿÕ¢à¨t?Ŷ"^Hœy?£Ø*:h£«?æ¥ÍIã6?¨¬lM^è?•å4æMy?x¡e¶Û?ÞãÀ;'	?²Ú:¶,Ø?ß½ïq'œ?²{ÿ‡h¨4FGL J1719.1-5348¿ïvi?x²À"¤w¯dÀ:hRGËp¬À<¿¨!Ù@…"|NZ+@–žh5s?¬Gq-À?@‡1Ó?Ñ´âË;Ó@×nŽ¨ú¶¿îJj½
<)?ïò§½HËK¿Ý·DdÞÑÝ¿æ'Ê !Èþ¿Û#¾…â-¿à9"¿ºëyUNASNone?å›Ä¦7š¼?Áƒh"D?'+cXö?‹G'D¹H?ÓµÀ~ɉ?ÁO]Öñ!?éü/ähV?Ç/ÿ C?Sƒ(†™*
?fõ‰Õ?Çè:PÐR?ÆÿX›ˆ;?礆ÍÂ?ªŒˆÛÞÛ?›3Á#ñ%?'–vàÀŠ?Î	=ÀJÕ?¨›!Ñ8.?ëëÇ#¶?šó;ŸŽR^?ƒ¬lMᓶ?t«Šê»?¾,:]*ÿÙ?šwÓŸ"/4FGL J1719.3-3424?ëü¼‡7õÃ?û!Â]BÀ:d%B{¦À<¦Á Hà@ƒžçŒ@Á@ľ
'*?ՈŽÄÔZá?ïú›ýwª@'
=p£×@Âè/SՕ¿ä‡Úà
í¿Ó§üÞ¸\¨?äz؍Út¿äém
A"¿ïüª£´P?ï@ôQvYUNASNone?¥ÎÖçž3?£¼2â´t?ڒ§,&ïŒ?Éô§‰[ªF?áY¿nV?ÉÐAâ?¹HÌÒÊљ?ÀíY%ýÿL?×þEðü‹?Ѧ—t£?à×Ãm(`I?ÐÍ̓º?Ð7vP½šˆ?ª©­è£~?×_&LÝü?²å-ˆò?Øicc>‡{?®ÏT¤ŸúÃ?Á½íï=Û?°eiýÖX…?⺚:^¯?ÂÖìV9þÊ?Ñ«Õ
L=´?¾"–_"ß«4FGL J1719.4-2916?›nÿ†Tç@n"$咖À:Q'l~®\À;UÎ{"¶
@!uÇ,yÜ@E¦'¶(F?Öââ7î?Þ¡x ¥§o@ ˆC0y@YKË°m?ïR…sq礿Ý]+4¾y¿ç˜Æ‰ˆ*¿æ¡^X¿îÚÑb2Ð¿ïþ*ÝúºUNASNone?ÉZP@'¼é?¹'2"Ÿ?̄kñâöð?Áhgá‰ä¶?âˆPób"
?ÄEãµuÆ°?ÅÀïk¡…Ã?½Z¦IêS?ÃÝgD6Y?À̺'ÀÞ?嘃Fú?Âu™Kÿ@?ÑÕAÀkŸ?­ï®lº?ÅCs±cD?¤ïF6Øay?áĂ\×`?°ÏÜý‰?¼•ã^W—L?œÞ{cö¸?¿TôW¿6ù?§9íù½È?肥	=&7?«,¾‰9Î4FGL J1720.1-4358?â
ܞ?àZÀ<Á^ڀêÀ9†¿:¬¤À;$G4q÷"@á›þMÎ?@…ÜMsP?Æ[yMsÑ?ºþv½÷qç?øýÎè/ÿ¢@9öw– ?ë0¿e†?ïx5›Ã?…¿éJº¾­OY¿äËZ;µ¸´¿àqÁŸ:¿ï¾ÿ—$tUNASNone?ÂM?¼¢€ü?µI)'¬ó.?'ïÐ(üîR?;e¾…K?êÕ1xO?·"Kݗkž?ÒÙ¤¹+»¾?ÂV4ï+i?'øóÏ;[?±yýßýŽ?åûfM¨F?®§Ë'–?Ϟ²û®ýì?«N¢JáqÇ?±êio»"?'ˆå'¥œ?åæUóæI?«Ôš‹P:'?֒~Èå?¯™í¦1²?´婋áq? !&Nâá?â4'Ì_?°Xˆ—@³4FGL J1720.6+0708¿é‰§wíf@7kDå^³À9×Ùµ›äÀ<àŽJ°þ@´fêD×Ë@Yܚ )×?Á#Q(f¦}?Ù é¤@ŸË':)Ç?þ¶§NŽ?ïý$ƒmj¿Ñô;[uǂ¿áäÊE¿ç|卍ó¿ìÞÛÃ	Õl¿ïä1‹@UNASNone3FGL J1720.7+0711?¥ó™¾"? ?x‰Êµó?çÛO‹ñ^?Å[]ʀ?ÎË©Êá?ÃßÚjÕ5?³\¶Ý7?³ô£"^°?ë¿Aªð?¾ç™5IË?´ŠK(ݤL?¯BªA½,Y?²?O-g~¾?™1,3›<?çQJ"Ü?°$­Z&û?ɛ.@ÐE?ª
"Ü6›'?Á<§ÿ'#ž?šZ݇#ªT?à4RtAΆ?³ÄõhôË?ÖùèÑ%?±Ï<¤zX4FGL J1721.3-5257¿Ýb¾"Xo¶À"AiÂ;ySÀ:%ÛÞ¸‡›À<$"û¥'l@
5]/@ô·Í?Åï"77y¿?ãªØ¡e@ëÒú
w¸@Ù¡û½Ñ¿Ï2þ'W¿Ý×&¢¬ì¿ÜëÀ š¿é_îbHÊt¿ïôù è­Ô¿ï%m
ÊUNASNone3FGL J1721.4-5253?Ÿ¶GǦb?¨ë‹!_¸.?ß#²•Ñ d?ȤûÛPÞ[?Þàèí½u5?ÈZÖÉòh?³˜#G"_?µ§FDr1"?ß7ÐS%#?ÍÛYB!Õ?Ü¿]ËØÅ?̓µ‰1n˜?¼É{ýýH?œºÕS+•Ò?ãäߺ'CŸ?±íÐ^Ÿ?Ñá‹^51?¬…Û<h¯?ÁR	L+‡‰?Ã~ÉüC´?à#Öån`'?²A>hb=X?×M
{î?°Íþñ²ü4FGL J1721.4+2529¿âó]òÆÓÜ@>?§e47?À:sÿÜĒÀ<DTž½ÅÉ@Œ¶¦Å§@æù[¡†?¤#
q¿¯—%ÿv Ï?å&-'2ÂË@ú 
÷Õº¿ÓÀŽ%D.¿ê–-žž¼¿éÿ7T*$¿çñ"'›¿ãæþÜêQB¿ïæH¿™UNASNone?ï¥Rë't?ˆ÷¨—âKZ?o	¿KÏ«R?t:èê ì??}ѪÚpb?'Ms·ƒ?ïbsçb?'‹ˆ¯°x?VîDÈ£\?fO>ÙD¥?'?
[–‰p?´?×ùÑ?íÊ
4ºNG?"ØsÏL³!?ƒ*vÕñÑ?r4F3®¯ ?®"¾ÿ_?'M~dÌt?ïl\=‡&›?z-RUg?l›˜ ·?a8áïúIL?Á‰¸R?w)òžÆ4FGL J1721.4+1131¿×ÉUSÄx@@9$ƒÛÂ3À:Eóå?ŠZÀ;íåf ÆI@dˆSöø@('»0Ã?Ä\|,Ì<?µÛ.dlf?ñúÑ!Æ#e@Ley+ü¿ïä:Âs­w?ï´êB~¸¿â7¨ã¹x\¿é¡nD9Q¿Ü4Â_5š—¿ãƒö.Åæ)UNASNone?íá9B
?¬Ÿ€vÈç?Š1umŠb?"ìhrâì?´ÚH"¯¢?«W#k‰?ï-‰Zq?˜4°Çcq?iáù•?t›6P–g?œ~-U{nY?•0
§׳?èîñXNæü?¬`ðѪÊ?£Üä'ÔI?†_Ô¹…N?ÇM%Ÿ®ÿ?©pùìNø?ëÛs9›I°?›RþÑÁîš?'‰RýÐá?ƒ	QµÏ::?¼'s±z?™†Dèœó³4FGL J1721.7-3917¿ïÛ}ä ?T¿÷ÝÚ;JXêÀ9Pè0-À:ÝîgQGñ@•8"Djé@7褙§Ü?ãRÿ" ?Ð÷Šûñþ`@À ìߒ?ûË …¸Ò?çi·ßTä´¿Úzµ]šdñ¿å^ê–p¿àuT«Rÿ¿ð?ïþ¥¢fqÏUNASNone3FGL J1721.8-3919?¼|¨Z…û²?±úe¹:?Çê«6¡ð?¿È^Me‹v?æuÀ',X?ÃF磬þ4?¶*Yˆ°¿?¶23ß?²úMù (`?µ(?lŸæÆ?êÛkÙÜ?¼Î?ç Bë?ÄßZ¼R	Á?£ZæÊÀÆÏ?ÉÌÊvß½?¨0§õÚ?äTöÊ
Å ?ªƒ9[œó? bg°¶?Œgñ՝`ª?¼Œó%ˆøƒ?¨‰£ƹ)?ëh;+3ßÅ?«Vñ¸t‡ù4FGL J1722.1-4007¿çÌMyÿ©À*¼¤¡5À9q¼´i)À:þX"»@=ó~'W0@µiF·G?Êl‡"?Ŝ¢x†0@Bõ:ªú@ͳ\cX??âøC]¢Èl¿ÜQ0^ƒ¿ä¸Çâ'@¸¿âs,þåÑ¿ïOÙ\'H?ÔVˀœUNASNone
?©ê5è­?Ÿøž×Ë/?¡œ×"îŠ?ŸBþ·Rü?í_52Œ?©@%ÀYÈ.?Ê'WQ‹7?À•1'T˜?–…VÅFcÿ?#\yEË?èÇpôj?À«¶@ÀPã?ÉãoWÍ?¦Ê¸ìÒæÖ?¸ûõÁ?— JËp•?ægØE›‡õ?¨m<ç&S?ÇZâF%àF?¥àþ'œ³?§¡ƒpðg?üUgU]?è¯/7gv?§'ÆÃɌ74FGL J1722.1-3205¿í'+årFU@Mt­P0À8Ù¤K¤CAÀ:³*dW˜m@ñ+:ÁG@ø¼²£V?Õ²½?É[¼>_@a~4¹E1?û/-4k—~¿ïr> wæ?ïýéÚúŒù¿èÄ¢'ßܿ䅠ž²´¿è)ó¹  ¿ïÿ´ìw8UNASNone?ÑìkÒL
L?¿gÜ´–è­?òÞtšEo?»—M®›\?ây³gþ?ÄÙb'?²€üêw?¯`¸Á;œE?׌–¸bõy?ÊəbÇò?á礢îçõ?ÉòwÌ÷.@?ÈSoð‰
 ?§yV¥ê?ÃfÏÅç?¤‡
`D"?åpcø?­r{÷ð‰ô?±:®á
`?•{³8Gá?Æ1dS
ö?¨«Ç¹i?èLc
È»6?¬Æ!Áä 4FGL J1722.6-3135¿ïå¦åd@¹^ƒCÿÀ:m^º z^À;üVÈc±€@XýËrYº@Ú³R¨D?փže[N…?îù¶9ãP@Z5Ö{¢?ÿ‹Þuk¼ç?ًÛk¡¿è×n~ÓE¿Æ~h»«<Y¿Ü	ÆTㇿïÿý{ÁA~?h$¬ˆUNASNone?²ËJ‹?±†Ês½?ÛªÉ«?˂[M¯ÍÍ?ß²:<c±¬?Ë¡¤¦?¼ê +ÖÕ°?»A:6P4?ڑNP?Ñt4?ÆfÓ?Þ4B¦ûúx?Ð+œ´?Ò}ÜÚâ?¬9µëø´??Ôö}§o»h?²áøB.?،y|‰i´?¯<"‡½ì?ªC"ËfË?™ßsÇ´:?á~rBÀ!?Ã14¹ø?Ùºªø¦Q?ˆH

4FGL J1722.8-0418?í¹b"·Ç@1z¿¹¾ÓÀ9£ÎµÛÀÀ;ƒ¤Ùš;@Žy&²qW@òÜ`¾†¹?¿È`g¯ù?ȑXJz@é{f¨«…@d]!Ä ¿ïúþ8£N?ïþ|¿á
Æ,Ÿ›¿ç?!þØb­¿ä…ºŸM¸›¿ïÿõMõVYUNASNone3FGL J1722.7-0415?ꉣ`¨?¹pÏ#Ë?¿yjd9¯`?µétHZ5…?¨|¡' P?£Dá8[ñ_?ä&¬¦?Í)]~˜Kê?Ï^I1Ñ?Ëa£_{†?ÀQKƒÍ?´¹Ðy›&D?à̔Îe%?±}áR10?¾ö&Ýå?¢aj/öÁ?Ö©Rƒl=?®¯4µ¦<h?Õý«ý÷×?«
.Ç!G?ÏQ!ö~lŠ?³	 ò?ÚYÃìÂÑã?°nm_&>Ö4FGL J1723.1-2859?å4•3Œ@_\ÔmÀ9áºu²3ÄÀ;U';&F¼@¤š"i©½@ùB%?Ò*5}æ4Ó?ß<eáÜ)@ÅSü×V"@ña£Êu?Öû{8…ƒ?ïäÕ!…
ì¿ç²™0¬¿è:P(6ï¿ë»¹.׿ï®
4»ÉUNASNone?®ô);±ˆ
?£­a@¿Ó?ד˜œ¿¤?ƃ=87Æ©?âFñ8­?Æ}Äö=?½Éþílâ?·î',!5²?ÖøXz?Éýk6SÉ?àʔFßÿ?ÈõM_ra'?Æ%z/yX¬?¥|ÆÁ]Ü?ÈÉ°í?§?ù£ÓL?äq¯.un"?°	ÂÏõXÏ?Ã¡…?¡<MÐQF?ֳɧæ?µŒã˜é¼Ò?ßTÙÍÉ,?³@@aœôØ4FGL J1723.5-0501e?ⱟk¯jU@0ös>»ýrÀ8¥½áw~½À;Gýœ@ sÍ$™g?ÿæI ]?­'—¾V迅'LmcR,?ÝÉn"æW@BØ(J¡å?Փë$%Ï¿ãÎý'¬¿ã©yámm¿Û1¢åGÂâ¿âCuÀÌcp¿ÆÑM$ ô,UNASNone3FGL J1725.0-0513?ä¿òõ%?Â.4áÍgÚ?"$_>N¾o?ŠÆНì¯1?ÕO()Ñ?Áïà1$?í•þóýN?°œ7Ú£Q?‹Æµá??—>Œï‹4ö?¯®cN¸Û1?¬Ä؍)?Þi>‹ï‹\?³ªbOÐ/?¤ΠáÙ×?ÁŽ®µðr?ßǟô9h?³[P?L]b?ÛazÙÌ?´P]oÑ V?¢³k§695?‡vϛ̮?áGˆD/‡?´_FpÏÁ4FGL J1723.6-4126?¸†•[Àž'6§À9È.5p¿À;/51:4¯@'')Â@8M[Óem?Îàw	KÙ?¿ƒ"´µÕ?÷ÞêÁªYÛ?ã×vŒ#d^?íu–Ob=ã?čsñidH¿æIÅ$½ú¿æ—:yx'â¿æ™Umß¿ÌD87SÿUNASNone?Ê"ÔÛA )?¿¾J!ë^¹?´
¼¥»Bq?ÈøN#—$Y?æõó4x/¨?È¿|;¡Ü*?ÁœKø%?ÀG'ïŠ"?«¿Æf3Ñ?³ǽÇ&?éÜ𛓀î?À©m¸ú†.?ÎÄûG›!?ªAºB]?±G-z>‰–?'0ÿo‡fŽ?æ%Û~Ñf†?ªߘ@ý?ªÝ'LÙhî?ŒJYq‡ÿ?Âóx¸2?¨ìE¦á'?é•OƒN;d?©@áDË(4FGL J1724.5-3008¿°RÃâN†y@	aâs'?À:©¹¢MÀ;£­X"?
@Oe/Û@Á=¼#1?Ónä#Ösë?íÄÿxñƒe@zbœ­J?úbԘôF?ï^ mÿ¿Øꁺè¿áæ">iƒ¿ìªx^¶n¼¿ïÿÿ" 5•?á3Ê!Ì®oUNASNone	?¢âe:°îþ?¡.D™]?¾I®LÜm?»(è4­,?ë£ékUƒ?¾c	€*û?·$<¸'(Þ?¿¹£èI¹?ۊ:8¾.n?ÐÈv¶°`Z?Þ¬¶™8[?Μ†'I?Â|HÔۘU? FÏë??Ùdü‹a?³#tiãp?ݶv™ÒÄ?±ŸÉhH¨?"t"´ÀŒÝ?}qÕú‡îß?âˆ}[ü¾?ºòRÚéA?Ù¸žÙûý²?º<Ãg0‡&4FGL J1724.7-3737?¨Öåác¿ð¿Ï"èbUÀ9L‡?$>À:Îr«G@O²{<â4@YH;4Ž?ÎqUää?Þú™#R @
.9™~Á§@rx¨ˆIæ¿ïâ7,¼÷m?=î"2¿çù҉¥/пèsGà¿Gÿ¿ç!ßMØÑ¿ïÿè2_NUNASNone
?ÉëäóÒr?ºÝ{?»ôô?Ä3÷u[?½
1œ ‰?䭇Ee´ ?÷ø~Ø?¶z°Ðñb…?²Áúì4"?» 5mB?¿ú³ÀLø'?èæ=Ôx_?ÂQhܞ©?à òrçÓ? ¯
ë{´w?ÄoK[J»?¤+-I!ž?æ7›ðŒs\?©?»?"?¸A)uR'?™åý£7]6?ÉfT¹Þ°Á?¬_Peå/?æžE¢Þ°?° å"4FGL J1725.1-1924?èwj¼SG@"ˆP›ùÆÀ9Oç"!°TÀ;‹M@$³>@FíùXŒ@_ž£Ä•Ç?½uQçÿƒ?Ê⬩@3ٛè(s@@~æ?ïýüºÑ!Æ¿á'Ñß^¿â7Š`@²x¿äè‰÷e&Ë¿î鱿«&4?ÚD¾@BoUNASNone?™,ç¹¥s?´³)Œúì¹?Â}{6
ö?¹VÙ@Ã?æºUøŽ3%?À³"g#x
?ÍUÖ"pø?NJ̣`Ø?Ö²®	½¿Œ?Ì´88à­q?Ú¢fõø÷?ÊýÑ¿éy?Ù^Ú¸mã¬?¯¿Ï_Ÿ?ö?Ł	á?¥Õꉸé?Üd¸+È?¬ø
3±¸ð?Õz)–!XF?ª]ñrNÏ?й|äP?­›—¼—·ô?ÚnìúWª?«ÉÀ¦4FGL J1725.5+0840?í\}V9iû@7t>–=ÅÀ:8"ïïÄÀ;ø³ÓÃt@o‡]s@®^L¼q?Âv'ƒzÉJ?·4—¡Ç»k?ðÃmrÊ!ø?ûF°¨ÿ¾¿æáÀå7ý¿ß©jÝn…š¿ë¢†ÝÕ2Í¿àÀœ2#i¿ïýR¦–_¿ÝŠºC2YÄUNASNone?m1‡s?ŒÁÉùßæ?e"·u¤ž?‰|3,Êý‰?úè~?Z?—э춺?ìª3ÌWŽ"?´ÓË7pY? E¤±ª?¨Ã$ˆNY?²g¾Ë82"?§y¿¶Ý'?èéü#˜—Œ?¬#pÌó°?®~¯pr&!?›™•÷?ĸc•D?¦?XÜÄ>?è¯Ñ*̊R?©Ü:²Y?´4ÿ¸å`? m#*'"?Ã&;xÅd?£	£`¢Æ4FGL J1726.2-2903?ë«ô«õ"@'cj2¤À:3±6nQÀ;x'æÏ­R@Œz@ÎÀ§¨?ÒD@ ×f?ܺé"Ä@	Yšäó4@e
˜ÄÝj?ﶋ!±«‰¿äÑï¡c¿ÁáBWC¿äµüŸ|2¿ïýX «Ó¿ì òʍWUNASNone?»©*ߙ)?°ËîryÈK?Àýð
6w?·"L¦ë›?è"(	B?½Ð¥¯¨Ü±?ɌæŒuX3?®o¨=?Á(ªûgª?½–Y+(
?åR›ÛãÐ?ÅHðB"v?ȽÛ§ÂF?¥K®¨&^?LJXfàò?¥|³éæã?ãî³Þò?®Ÿ"7ô-?º"»Äy ? ]íh´ë?Â"-d€ª?¨yr¸¤?æÈñµÁn?¬¿|My4FGL J1726.7-3930¿î·Ïæq–ÀVq¬ÆaÀ9ÔÙb…UÀ;>"à4ê@>=I·™@¶
~C›?ÑkøvžÂÎ?×(Õ_°@Œq'êS@ØéÆW½¬¿îo<c]j?ïÓpöa7¿åƞµbLü¿èÕ·UlC¿æ¶9­ ·›¿éàbiªUNASNone?ÎE
˜ß?»Z4Ës?¥"($? Ïh@&îŠ?çóWEý?½òBcT)×?Ċڕʱ7?»ví/‡á?¢ì‹642?§XûñµXÄ?鮀§*ÿ?¾N†7ªÐ?Î1ÞÅ£›ò?©Ó؊'ï'?¿µ›eÊÁÓ?ž#v~^
?ä|ÔáÝÀÉ?¬ßÈäô#«?Ð#§°zЧ?¦š.VØè¢?³È£Å—tÕ?œ7	Í«BZ?åu¯©?ªg‡1«"ì4FGL J1726.8-2659?ÓjçÛع@$ý£.mÒÀ9º`@²w·À;_œÈù@Bm¬@<eü´%?È÷ùñÉ?¶éÀ£s¸	?ós̀v²å@ýb–Î
?ïÿr ®Ì1¿Ý§š
\à¿ë'ÑÀ§zƒ¿Ùµ'm¿è1B}Sö¿ïÿÿ&¦³UNASNone?ÕEöà0±Í?žhä×D	?…6Sl&H??£A÷Eùs™?å+B7
ù?Æ¥¢øæZ?ÚnZ€T¢Ö?Ä:Œx0?—'Ã\¹?œÆ^(ÇÉ
?âÖ©½¯?ÄÅ÷­â?×ó!}?±
TQÓ*´?±›^}J»¸?"ËÆòÅ?â>¶Åê?°ìåó#2?ÙuäF?²œ0™©?›˜T>¸xá?ƒ%^g®™?⡂kÁü—?²ñõW\<4FGL J1727.4+0326?ÝGn=B'@4:GýœÀ:5N`¶#=À<§Š$Ô@˜ŸBÐà@ —ºœH¡?ÄOI¿;¿Ÿ?њIâøc@V1µ"±«?ùÝ£í¥¬¿ïÿÿ>¹ú?ïÿúŒ—Ó¿ÕÜýë©¿è€#¦Î6¿ã(Hr_™¿ïöÈHٍ¥UNASNone?è¯î¼½w?¿™Ú¥V>?¶'úP|c?±œp·µ;Ê?Áù±á‹ö?ºC:\7?※å°X°?ʘGc´—?Òmž!!R?ÉûUôŽ@?ÁÒ5,üZœ?³3S÷*û?äf…!TqŒ?°˜´•(¬«?À[)'i$?£˜w‹#¿?Î
ÂlЪ?¨'ÚƼ0:?ÜæüfË­?®Ag¤»Å³?ÑUÊ¸:ö?³…÷*ê?ÑÃrÎ|?«ò¦ù*í4FGL J1727.6-2304¿î3=͞Œ@37ÿJÎZÀ9O¹ã»ü›À;O¹ïzv¿@åªi @hLŸëÃ2?¿šâÑF?Â½é:ø@€¬:†
Ì?ÿ¥ì©&¥?ïò'íÓ­'¿ç5÷¼d ¿âµ{A¿½ñ¿ä} ½ê¿ãG ñO´¿ïü&Å¢·UNASNone2FGL J1727.8-2308?܅#²(Vº?ÀßPZªF ?¥屘N%?Ÿc{ëA?àmËÒOÁ?Á9ŧÂ3[?ìö«V¹?¹Cl"ŸÞ?ÁGžm,8¢?ÀK™³QX!?æÂÚÝJ)?Á'ì67Û½?Ûùd­Ò?±c±¨VI?±aôaŒ?"¢–îŒÎÂ?àQDïʜæ?°½þ!–ãu?Äh¾+3á?ž(Èk–Œ??»Ó&R'=-?tbÄØß
?çÁ"ëb?¤‰c¢ñ4FGL J1727.6-0849¿é›Ð·×¶ú@,LÃ\á'fÀ:=LÖrgüÀ;€S`'@ø%ËÁ‰ù@£Ho›?ã/`•Áô?âræ§if@
D7'MLº?ýÔ(ì]`Ù?î'—L¸?¿Óx™q¤ˆ¿åëi~J‰¿çžb¿ïûh÷:^¡¿íòá~µ'žUNASNone3FGL J1729.9-0859?Ño›£Þ|ø?ÁèJ˒?ÔÇciV<Ë?Ç,ûl:@?ÙÉòËF;?Ç­Óô<ö¨?Öt7´O¢?Ð^¬ 7?ÙÑf©‹×5?Ò(:
êT?Ð%¿Ù)?Ç-ü*ü«?Óf÷aÑ?ª–m†ȵ?ʟ~»´m?©8[sÖ¾?ßJ:ªÃï/?­f!*=?¶!tk–yY?ž²ìÅ×?Éä3sDZ?Á†ž·@Ç{?æÂĕ¼¾?ÁFú'†i4FGL J1727.7-3621?ﺢ/ë*0¿êƒ©8sÀ8éXjËPÀ:6&æô–?@ 2¡'âE@j r}Ì?ù2«¹VÎC?Ô2k€³š@fî0Ê£'@ÜW·L?ïþÝ@7}›?Í.-ºÎG¡¿è¹]"?•A¿äÀåÙ
Lð¿ïÎ¿ìº?äŒt¸8ÁUNASNone?ÏÓúA…?ÄÙ¾‹‹³ç?Ò
P	±?ÌÀš·R«?Þ/c¶­®?ÏEçfÑÒ?´tƒA¥h?½Š¾þ'Ä?ÄU6¦Û‡ ?É3ºbT?è\!î&il?Ê--×Xµ?ÀA¹Ÿ§p¨? °uìŽû3?ÌÄÒ`3ÀÌ?®´pè×Ëå?ä¾]	3£?°TüegÈü?´0Ü?´Èmbà]?¢(Òb[¼"?¶?Êg.Bh?ì]ÓØ´?¾MþÙõC4FGL J1727.7-4041¿ê_Kg¡>À	ë9\B 6À:B–Ù˸ÑÀ;Š¶ÂŸLa@'KåÓª@yX`ê%£?ȈH8}õÏ?§[Õ=߉"?ãè"=ƒH@2Âô†Ð?Óì{¿¿éòH‡XNv¿èÁ'ïV¿å'ˆ˜ÀUÆ¿è"Æ@–ž?º3˜ôUNASNone?·l–Ý?©–1 Ñ*Ÿ?uY@+誏?pT1Ýæ¶?ì纣ê:ø?ªAS¯rèÄ?Ñÿ"ƒ{°Ë?Ã#Šˆ/0?€ÎˆÃ)°.?á@,¢ŸÔ?æ¼ü5€Ú?Âàj3ó|?Ö+²'Ù-ç?°Lö¿§ì?§‡(ÐCå?…ÃyëÆ
A?ãxžy†dÎ?¯"<^&??ÕMAFgï°?­µ7<3cÊ?"qÁ‰uƒ?'™;'ÁŠÂ?ä½ÑP|?®pØ4FGL J1728.0-3550?îV:ŠH ‰¿âÅuà¬ÓˆÀ8]qHA¸1À9óÍêÙþ@,³ô8Ìz@‰µ/ê©?ǃԠ֤½?Ù°ì1"@ªàéºC?ý­¼ÌN¢¥?ïùÐfqN¿Û™¨G²F9¿ãpöBˆ¿éÌòŒyöf¿ídÚu+ü¿Õ£ãßãÕÓUNASNone?…ÒûÕMªF?ƒZ8´
?'?«‰Ñå?•?=†½wý?ﶷ¾zÈ?šçz+8ڊ?¥±ÆìCE¯?¤
ŸšÊ°¬?Æ÷†Á'C°?¿àµƒ¨?èçà×:¸?¿Ôeù³!?°naa‡?OȤ=&?Äèxê1{?£åxÎZ˜h?è´42™B¾?¥ïµ°?wânödá?eÛA¢¤?ı}NáO¸?¬1ºv,)n?ê¥bçi¿H?¬å"m$üä4FGL J1728.8-5131?ï_ ªº~À"\ú¬ÙèÀ:•:a%À;ñ3eˆ@'hC¶86@¯n'"šV?Ũ%$&Ñ?ƒEÍê"Ò?ÀÇ?EvW?ÿfwM"]p?ïCE.Þ9Ý¿è¼ýÇ%C¿æì€üê¡Ê¿å)	
Å»a¿à[BEÈa¿Û|M"ȁäUNASNone?à°¦½v‰×?Å(p.+ªþ?z_×»úŸÁ?o"e§–ž?Þ53&#Ó?ÅñoTÓ?⋉ù£ò?Ê!©#žÕ?pÏΉ•?~ÇJ7éÝÆ?Ú¨â´Ò'È?ÊÂÍ)ò?æÈæ3¢x?­ š¹Ÿä~?›
X3ïC-?€b~‰ÓH?Ò#È°YÆß?¬>ìn6Ùl?éd"Ô"iý?£wïQäy?ƒ•ËB2×V?rLt¢'?É4ûS*˜?£4P4FGL J1729.0+6103¿àVÐ;
¿~@@³¥ 8LÀ;H!ÔfBÀ<•>zW@moe©P@³ê-/ãó?ÕÈ˒:*?Њ+<™¹O?÷åþFÂ\1@	0=Wyc™¿êë?{@¿èb¼Õ"p¿ãÊHŽK¿èìóþê×$¿ïÕ»Ÿíq¿ðUNASNone?îÿõhí²?À3Ê…?™õÞ:ôý…?ÀHꅕ³3?x-Ó	50ñ?tú^=qŒF?î¾ÒPæž? ó<Ík§Ê?q_zå¨Yb?'Œ«áOr?¡æïn<‹?œáÀJ¾4?íe0‡Î·'?—ŒÐûS?"A]ϯ̧?"™Þü/ð?¯ŒH›< œ?'¼Ø(ã\?í›õ‡
ºD?œžˆÖ'C7?uÛ·3ÁT?n…ÃØ/?±Â˜Tn ?œ¼Uê"54FGL J1729.1-3503?Ý‹pa¿Õ_/:€.À8Ý6ñLÀ:XoÌW@Š
Zvï@QÛèº?Ç¥ÿX:?Õûò•í=@Ç7ƒ$O@ƒê÷Ûj?çÀ;Yrb?Ô¹¥¨›•¿âŠèü®<¿ÞÛ	í¿Œ¿ïk›Äí{¿ðUNASNone?‡›¢åíã–?—aÆøçÒ¨?Àä8	¦Æß?¼DšÇŸm€?ëhƒqþ–º?½'`ÑOï?¡fƒBí? ŠÓ3®L?Å̃{~ÁÂ?ÁÆ¸låq?év~îë`?ÂuLŽmc?³")R{?•ú²(vQ?Ó_-Âx?° fC.à?ä‹K¦ob?¯ibù?';ÓŽ@¢?LÆûô¡´?½àÙðƒ?«óc¤Þ·?ë²)pKê?®µÏèU"Ê4FGL J1729.2-2509?Ô-Ÿd@^øÀ9â"Óa;"À;3Ï`ûÃ@!/z–õ@uýfȌ?Õ6»©?å)Á¿þ]>@CEÎ@j?û_ò+V?ïÿTsõ›"¿ádpݸ­[¿æ}Kà~/†¿ë™ðlF¿ìV¯°¿ïÿÿ)@k*UNASNone?Ó¥€Ö£I??ãlÚ]I?ÈP¨؇?ÄÏí5€u?à§å>?È£«2ßHk?¸tNÖòéL?µÓºËn""?ՔË\)ÝH?Ë=ñ-?â'w´2?Ƕó?95Ë?̟gŠ(,?©Mg˚C²?ȼt%?+A?«å'R&–È?â©	&.d?±´'€—Ù3? "^ÜG*?Ð@"õ/ø?×<֐֬?´déüRÍ£?ã`¬q¦å‹?³öyxÍà¯4FGL J1729.4-2831?îŽ0Ä1âj@	È*ÜLœ'À9¸ª½®KØÀ;_ÐJ/Ï@-ò»ô¸N@m.#(ú?ϝúé×?âÛÛÈé~@‰Æ×p•?óëà;§R?ïÐ•¯)N¿ÙsÇwù5á¿æ(oÀ';¯¿ì6ĸ+U¿æÑôSúS¿ïäîâKd,UNASNone3FGL J1729.5-2824?±-°pH8œ?¦:åÒý?¼¶lOÓ?¹h‡ü4n²?êJS"	nò?¼òx@¨LZ?¶ýÐdµÃ?½ÔÂz©FH?Ò{kš|V¦?ÌRlm¦rÁ?ãâ§xµ=ô?ËÆN–aϟ?ϓ'—?¡bñW•?ʵ–Ÿev¬?®Öµý°è	?änµsá¼u?±sÆn<HŠ?‹ÔÍy*?rnÛùâÀX?ÓLÖZÅ¥?´;ÞÍ1.Á?åêDÃisÉ?´G1'êš4FGL J1729.4-2646¿ÊqNnDx¢@¬¨ââ¸ÇÀ:`{l‡è—À;ˆÌ&°n@û8|É)T?öœøä'Ëø?ç§"ïQ0?꡵A•Ì…@Ãà{Ö:?üôRÝÊ?ïÿð懈ö¿ë$¦=¿…ãÑZÞ¿å_ú†C{¿ïÿŸB%‹¿ïh‹9"†UNASNone?¤Jd¬mÙ?­ƒÞVF?€JÝcg?ŠòL0"9È?îz.?¬ýö?°Âe!?ÓjÌ?Οf¬Út?¸jüÂ@)j?Àv¼0Œ?ãjkf*È?Î8ñ;+ó?Í5ÏTCÔ?¨äŸíFõ?Ï>e|Í?¬™îM–%?àãÑ­Y×?®Snó<9Ý?ÿ*ˆW-?¸)|á:Ë?Š'±Zqá?™ÑÝÊ̓?ê¦*˜"¢®?ºßÍwϤ¹4FGL J1729.7-4242?ß4ÂcÙÀ–Â&€IÀ:71xH:À;£¨z-@&‰/=õ@Q¨òÓ?ÔòI~N9Ÿ?äh¿µ<@‰å\ËO@íõ!È}?íD¹ØÔB?׸ÎG*a¿æœ†é"¬ñ¿é‹@•¿ïKtÝøn;¿îÁ†b…0VUNASNone?Ѝ¤ ¢?Âíé~P~?ØÞ
ŽCò´?É>ˆb¢ð?֔ëÍ:lª?ÇaNH"?»÷	¾èP?»EQtY?Ò¡'¿Å?˙OÌËùü?ã0ŠèžÁ"?ËJ³±µ>?ÑÑäíØ~ƒ?¯}Ö~?Î<\ì[C?®óN×Ñû?ßì›ùòÚ?°bX¨3?ªÊ•¼é©?'¬œX‡ü?ådåõkäŠ?À'5Þ¸‡?ÑÜá]‹ö?¿à*‹3ah4FGL J1729.9-4148¿Ð¯9.òBÀºG²À9t(<æÀ;g
"fy²@àn"0žÙ@՟Ú%{?Àu	l?·uPdˆr?ñ>³nW@Ç'¹ØSi¿ï·б]Û?ïÿ´Jõǘ¿ækÑ	ro‰¿æ'á>sÙ¿ànw¬ßÇ¿íBåøí½UNASNone1FGL J1729.8-4148?åJ7!3·s?À« »&þí?ŽõÐj%Â?‰­lŽÔ-?Ôsã:Gh#?À'QÃyz?ã'vâ´¦?Ç š\6Ùé?mp6ªÕðO?{Øätbð?ØÀ1ΈêÓ?ÆùÞ·Çxö?ÞaÆ~zï^?´"ئ'¨Â?®?3æG‰*?"ï&ð$2ž?ÝÖS¼{?²«•«ˆX?æʋëÅîÎ?¦ÿà"A?¢l÷ô{=Ý?}´†1;%?ÐI)亩?¦-fÛê³4FGL J1730.1-4343?ï'¨æiÀ[ÞM'ÑÀ:.¼ÆÅKÏÀ;¡=ȸk@ª|ÂqU@S°ÄXŠ?Ñ°™É=v?é(¶!å'ü@^(}ˆÂ@¸¢kOYZ?è–Dzƒ?í`ov°`…¿åú´f¤z¿ïý»aëW|¿ïí¼ '+"?ïƒnI‰¶ÎUNASNone?Û¥jk‹'?˼»¯Ë4?Í`h'/ø?Ä
‡ý7?Ö3Pá€Üt?É}Ûejèš?ÂV°ÀŠ½ì?놫£0?Ö¤'Øìš/?Ð*Ýë÷¦O?à
cgn?δaG…œ?Ìâ3å¾á4?§¼»z;È?ÓÒ¬ÇÞê??°—-Ü6Z?ݼ9EA¥'?¯¸Êóê®?³8Ï?gË#¿{?äžÜÝ3æ·?»{˜¤$?ÑހÀÊ/^?·ß¸ŸhC4FGL J1730.3-2913?ïzÒ>Ú8ú@Z¡ô±îÀ:Àk<ŽüˆÀ<Y<Íù@Ã÷h+ã^?ÿ{xFbºà?Ö·Tà¬þ{?ïÿp=½P@¶WuÇ,@‰-Vû9r¿ïa.ƒ¡	Ð?ïì­"šB?¨o‹þüIè¿Ó¼_vÞ¿ïÿÿ>¹ú?ï߯BxJ"UNASNone?Þyî¶]à?Í$B~®?ÏX™ÄûT?ÇAUF4'?ÑÙÄ»$w?Æq±Ä7s?Àkâ+  ¨?ÅLK®>®ì?à8¼q"?Ñ©@, )t?×YÚÀ¶Ìƒ?ÏÏs<»>?Þ üpB?±|[ªëÓ×?ͺ±ˆ"²;?¯mî§ÐpH?Ó?M" ?­¶%šƒ x?ÕãôŠ¿Î?»SÓµõÆG?Ýè_‹UY‡?Á@æö5?ÈgXè?ÍV?²J-ÿœXp4FGL J1730.4-0359?ä-íaþÞÔ@/ý™gD²·À9¡ƒJ¢»À<	²öañ@ûŸZMÔI?þ´zuçãª?À_©]ÜÕ?áp'S­Q@B¸A$~?ô˜0m±v¿ï´qV"q?ïÿÔač¿Ãݨè)b¿æ¶ã¡¥¯¿ì´/GhG¿ïÿûÞ]BüUNASNone3FGL J1730.6-0357?™Ð‰"¹?—uE¯qu´?îr%R?­ÜÇüë6?˜°*ŒL™™?©2$E¦.ß?÷M	NÙ?—7V"?îÑÔ-
?°uàJ6¯ö?§!¤éìÚo?ªÓçŠ>ŒÅ?¤÷éßUk\?"µáÊ=×?ëvò ò_?¢ø"ç
-?¹ÌvÂR?bä[?–—nl" Û?€¸
-Í?ëf¿̅?©'¦ú¶Si?¿$+?§U´Bä4FGL J1730.5+6018?×ñ v'"C@@¡êhìSÀ:ǀõ]åŽÀ<g;.ª7@:ê¡tˆ@øåY‹?Ì<"1/?Ç£&
UÄX?ùÐéÅ@X—)§Ä*?àℏFY¿ÏRôčŽ¿éo6žø~+¿ãWB\	¿î{bâMg'¿ðUNASNone?íÙ7.Še5?§¼ô§&†?›õ(°´dy?¤Ù 2Þu?¤qø¾ÿzu?—ꣽ«›Ï?îy
Ï}_Ó?ž‹–"Nk?|ÒSŸXë?€—‡³?¤Ôؔ>åd?š,ÿ'q-š?ìr`Éç÷R?ž[.ïGõâ?GšŸK?‰íP7¥ªI?µ(§Êr¬?–λA}Âf?ìÇя>\?'BFݏ?¤þaðÙ?†¼«	rúG?¯r´…ú)X?Œ¿|öÄ9	4FGL J1730.8-3806?Óäÿk÷~À'¢&0À:@[9âzÀ;šÒרÈâ@LR_žK/@@þ¥Œìã?Ñcêöƒ|?㎻ßê‹Ð@ÊeI/ôº@AæŽÿf?Äöë¿Ý—Š ­_¿Ô«ÉGNÏ¿ãÀ'¢Ü8¿í"rmÛ¥®¿Ý#ÌbïŽnUNASNone?†îG"UÊE?|Á$Ëæ~'?ÈÕ
iÁb"?À›I7Y>?éo‡>P5?À»Lf8ÿÑ?´î'Ö'?¯Ê€ðk.¯?¶ÀÍAÎ+Ê?´[›(ï'ç?êŠ4Ëv´?¹*Ã	\³?ºPíZ{?™Uµ*Ôð8?ڋrž?µªÔ·>.j?Þíù&(C?´
ØI-À?½`½ƒIIw?—'c³B'?ǹ–萱%?¨ªl—?æe'•rªˆ?¬Gå¨(º4FGL J1730.8-1123?émËxÉQ@(EºÓ¦âÀ:´Ÿèh3ÆÀ<†íÅjÙ@!OµX«h?ú‡ºt´›?ÕD[å$x?ÎJ>ýìªc?ñL <K	ê?ÿvà.~m™¿ìhûl‰?ïø ÅÝÅC¿æN'à¿±kØ@Ho…¿ä¸
¾
¿Ùj"‡0áIUNASNone?븘];¿ð?µmߨ"b0?wÚûדR?p¥=®°)ð?À^ƬTcÚ?µ¤7¦^?í¼lûࢪ?µûQû,,?kPyäÁŸ?v¨¾ê"Ý?±BQÙìŸ?µ¤M'ÑèË?é¸ZÉß±d?ª!‰P"j?œC'«?Šæ™Ñ{"?ŝ,x\E?¦Ûhã¡?é±ÉÂl?¥ZjXŒ¤?‹mÐù~D?Y¹ÌÁ`?NJ‰ûæ·¢?¥=	ÌCá4FGL J1731.6-2904?ïÐ謹@("[CóuÀ:Î.äðÀ;cä|캩@".çßCr?ÿ´o"͊b?ÇB]Þ¨w?£©Þ
aظ?à¹¡Kê?ûë¹Èä
¿ïø…'‹`?ïÍ/(·Ä¿Ä û¸•Ó¿¸Ôç"ŽuN¿æ)S¶`y½¿Ñ'ó—»HUNASNone?Þ¥ýH?ÅÆÁ=V?]/áY™¥?U'Áü+?àé•}¯+?ÅÅ!{ž›@?Ü1Âk!´?Í&gÙèӇ?c§?³?£3u"ø?áq-p±ž?ÌêÕÃËb:?ÖBzBfòn?°'Gð-P?§>Mí-êÆ?Evcljû?ãjÝÿù¨?¯/lÜw)Š?Û¬Ê8yÂ?³N_ˆìÈñ?¢'û
Y?"0ÂäVßh?á{2ò·Ê?³¡ÃªFE4FGL J1731.6+0630¿É×5]§Gz@4®IäO QÀ:ç¦3ÛϟÀ<oyÌz@§5ÐòKa@)¹à<?×ê6jX‹?ïÿæՌŽï@zy5v'@Pԏä¹þ?ëŒÜ­¡¿Ã;—Æ/Ϧ¿ê
@?‹0J¿ïÿCwN7¿ïäÚ_²m%?ïâiamƒ;UNASNone?îqrDË?°›…ßàE?¥"æÄKY?©DMèéªH?"«³¤.Ïò?›BŸ>3?ÛÕùÀ9?Ðæ)2Ž¿?ܙÄã¯$9?Òü²C²?À¨ÊE!·?µoT¼•z?æ9Ì
‹j­?°É'†?¬µ?Ã9z"œC?©ï¦^°–|?ÃßU¶M¹	?¤þPŽ»"[?Ó÷ˆºí2?ºSùʐ ?à@âÑE?ÁŠ1&À£?Ç¿{šUì?µ0&½¥]}4FGL J1732.0-2659?ï÷ØÉQº@¨5ÞßÀ9£Y#‡Ä…À:2K@]':ØC#@ì=áò?ÐàƒãÏÈ«?É=+Úy]º@ðAFm@­¸#®?áµ "µ7?ïøŒ8ˆÊ¿à0rÄBº¿å?þÞ÷¿ß'Øa*'P¿ðUNASNone2FGL J1731.9-2703c?Ñ`]•L`Ç?Á6ÕQBÀ?´òßØ:LM?³Jú8¹Ïk?ä±u:R†?Í3Œ!Ð?Íd	B?Á»«àøCP?³¥ã%.ÓÓ?´³X/N€?æ+j™^µ?ÃK[¹@b?Ï í¡: –?©`ŽN*ÀÙ?¾œIXGÁ?¡Ë"¤i_ê?äd;l±.ã?¬	Y<§?Ë:‰Ô?­¥íŠÖ^n?¨¼9Xñ+s?˜)]p+IÍ?ç°måNxH?°cÿuFs4FGL J1732.7-2559?á¾4Ô¦"†@ÞµÛ¿êÀ9Àg{9\BÀ;?÷ˆb9±@ÿ‡ý@k§áZùK?˗©jÄD?ÔÂfa³Ï%@
˽Tn?ùÔ«JF¿ïÙ˜f"³?ïþáòο¿äjd!舿æð,µÿ+¿ì®a&ák¿ïþŽ`€sXUNASNone?´ì¿°«¥F?«H)øø:ã?Â;Äú"ú?¹çn=CòK?èÓwkê?¿ß$Å~:0?¶åÉrµ¨u?±y"ЂÉv?ԗI¸$O?ÇÃS\?âסõ—#m?Ç
d"Ø?Á½±Õï×ü?žë´XÙѨ?ǯ{S$¢?§Ó
=ÿ?头µ¾@Ø?­6xÊø"·?À…˜ʝ?ž\Žà3ŸF?Ï©Iö<Æ»?¯å€Tª?ãôGb¯›ª?±ÅŽcXDÑ4FGL J1733.2-2915?暑…lL@@öÿÁßeÀ9(=5ëtÀ:}äÎv@ƒYdJWg@"šVWû?˱AÖäþ?Î^® º4Å@Xùã†M@èîüwŠP?éµâ¥|%ë¿ãu
¸A%¿æîZY‡¿æ@å£]h¿éßb"Ò¿ìu¦à©ùcUNASNone2FGL J1733.2-2913c?Âa"C¦7X?²~µãW€?Æ=fÈô"¡?½Kitˆ "?åØA|ÙMB?ÂÙPÂà?º"Ê"öës?µìp:)I?¿ÎEzÇV'?¿ÜZ6vI?賝þ7Í?Ãn¦r?{?Å)WÆ3ƶ?£‡)8mÑC?Àé¤4¼l??¡¡;[Dr?æ{ACóC?©I)ÅË	"?¢[W\ŽÎý?‡HXë_"ó?°щ\úÚ?™öÑJs?ìÖ°Ys´?›çI½K04FGL J1733.4+2235¿Ù–^?•0@:²ÙßÚƋÀ;k¬ºÞ¿À=G€ß֕@d@ÚÖb@ÚÂXÖ?Ӂ:þϾ?ïÿ4~ô€@Ù>½ªðÚ?ýCw£ûrR¿ãHƒýP"?ÄYbFò?ïùíÎ à¿çdU/¿ïÿۂr5¨?ïüQ¿æ4}UNASNone?Ùӊ™§ÿ?Ëþ-3K?àZÜ^©%²?ÌÞr_Ë6g?µÚò¦t2r?²P0^ac?Î÷$fƒ'?Ï–æœ?ä4ì'¼?҉‡ÞF¬1?¾ÓkÑ?»Í[<?ÒdÊô'?¶0µµÎÕu?áNwF?ºKËÐ×_?ÆƯ˜49Ä?¦heh[Yí?ÒZ%7?ÁT{Ìã?䌔ÉÚÍ?Äkï`HZþ?³Mñ¨› ·?§F*…×04FGL J1733.5-2950?î|mÌÄÎ?û»gšCÅÀ9–,­®À:í¡(TH@!;rò»Ê@âIC?ð±?ÊôþÑpË?¹6xð+Í?ô»k±)X@]¬Ùge¿ð?ïþ$É
$¬?ïö)óð¿äJN듿çÜÖÐ[͆¿Ã-ˆú:UUNASNone?Ñ;vŽ¾?ÅR)·™,+?—ñ¾¯Œ3?¢ˆÏswT?æ²TO<@P?ÅëŗÍsä?ݙµšKô?ÐyÐ#me?«ÙyŒ
?¡1`QŽí?à­ÆgAY?Ð;"Lõp>?ÎëÎü›?ª_ñ1
Ø	?¶iãMÇ>?žæ+ƒ–;?åwÏöGñw?«û6ŸQÀM?Ú
a€öEN?½sê<F·?›èL´D¾Ç?›pæƒÃ0?âÙâ·c?¾¨ê6ÄVÐ4FGL J1733.6-2431¿æô=Te@hŽ^Òô.À9Õ]z.šGÀ;s‰½×g@0™@
ûÖ¥"£?Ëæá õ?á…X'@-+Ç.'?ýÑ}3'–¿ël{ž†é>?ïùÒSõJš¿ÛÆ~1ß ¿ç"ebZh+¿ì&îRz÷¿ïðx£ÌiUNASNone?ƒ£îÜù?y÷Tž|~«?Ã5Pòh9c?½
SòVåN?êäCª}Ä?½ljØAOÌ?±Ðó]֜{?°-¼¶Í˜Ç?ßʖT<ë'?È«õ´L"o?ÛÁ,ÔMmº?ÇÇy@Y±'?¹ÑT±ø§–?"í6ÝdŠo?Ò¤çÿ±]y?²77¶Ò?ãsaiè<P?²jf8;SÝ?¸¼ÏJ°E?•òdØB©?Õóúg¬Ðf?³N}úæV?áîhâӏ,?´Ülú˜Iú4FGL J1733.9-2220¿ÞeGÉSÃ@℁Ú`3À9Ÿ¬îàóËÀ;#J\D¤u@TÞ»·¦ @óà{Ö:?Ñ,à]Î<d?à€å7ýO@úuÚw°;?úÞÿI¡´›?ïÅÝÖ´¿ÜGm\¤Æž¿ê³Ãp=U¿íHzøÄ¢\¿ïÿþˆ0»Š?ïõÁ%y·UNASNone?ÙÐyȬŸ¸?ÅÔé{—'?̓ؔæ)?ÄÙêÁ°E&?×å™ìàZ3?ÆÍS¹¥ö?ÂKÀöB]?ÂÜþmçÑ?×ë¥ÇHÔæ?Î&œû'i?Þîy½•üŒ?Êü%>ïz?ЍEÓþy?¬žóž"Ý?É®\]{[?­SÍt.›&?áM¢EÕ!í?±‡‹©°!k?—ÌG-¬?"¡"¡ˆz"?Öò@ã€?·úþãðËõ?ãš!,?R'?·ŽÛìé›#4FGL J1734.0-2933?ïÿïI#Št?üø[ÆÐ3ŠÀ:Jøš°ðÎÀ;ÿGóÐG@ ;<hfç@2Ú˓?ÖöÕ^ìŸ{?ï?CwN7@
º ¢¢V×?ýþ0Çóõ¿ïÿø="ßE?ïÿîÝÃÀ	¿Ú~ߟã5¿Ö¯£#Ûý¿ëtcˎ߿ï´ì`»×‡UNASNone?¤Ó½£Ãô?¦«éèæˆï?à÷{Ú?ÎóDoͪ?Ý3š>§óD?Í}œÆç?–Êñöœ?¢æš[ÓH?åjÏj²ìB?ϕDÒTÑ;?Ó½ÀˈH?Î`Ï>pœ?ԕTDÊ\7?¬ñ"±«Ø?Ñk‡VZmŠ?¯5ãðéÖ¯?Ùÿ$dÛ6=?¯;k.ud‰?¤Û/hÜCú?™0zâ"à?êTõÝT?¸Ä*BÆ¡?Áu`Sž¦?µO.E³?4FGL J1734.5-2818?ÜnSƒw/@[»èxûÀ9yÂ=ägÀ:ô˜"¶Ü@F3#îǞ@N¶Ú@¨?ÊöíÈ
˜?纽֏Ä@ð«†+(@úfÛ×+Ë?ïl-_ߎ›¿†ÏÊ¸Ëc¿Û«n®3"'¿í*__6p¿ÚŠ|›1[¿ïûr»UNASNone?Šö"ìMin?ûÜ·¦Êg?ÂIA/°hT?¿h¤î?ëÕ b°F?¿øÔá5`ñ?ÂéABº'?Å¢'6Wþ?ɜºE1¤?ÆÕëÇH?äށ,(p?Ë¢Bj?Á˜3Ù§@'?¡­
‹Æ	?Ït"_ä?°‡ÂAÅB?ãÓV	
—â?±-[0^!'?­b}°)<°?˜Å-cb;?Â!;¤Ãìd?³š®6ÒKp?顉;Ìq?¶^¶ÚHï4FGL J1734.6-3548?ÞDX"6¿úýª…z'äÀ9Žœ÷+°À:זߪõâ@ /§zùª@bŸYÌúð?à•
ÞÖ9³?£N
ÿòê?ÙOGß=@ú±Â¸L?ï¼Ü)a"Z¿ìe€Y¿ä¡¿½ð÷¿ç8° œB@¿î½©CZÉ?à'F¿,%MUNASNone?±ÉúLæe?¬L'€YÚc?*¸×æÔ
?¡ù$Þʝ?ìÝjï£ü¼?³KÜ«)	?Ï¿­ý+¾N?Å?¡d¨?€g1ÕæL?'UþB]?çÎwº=¸Ó?Äú4{f?Í[—(§=?ªº‰C3U
?¶å܃ÐÛ?›€¡³	È?å̄	»ºÏ?«Ká¯ËÁì?ρ­¦kÚÓ?±¡j›qSË?x$ª²'UG?|qä­0…ô?çïKAº ?±á­±¯Y4FGL J1734.6-2912?îŠ
ú-?þ2°ì©À9¯mO"¼À:À'\f2@!Jgö…`@`RP/?ÎË]k"?ª]TïÆw?åóø :G¥?ü‹Å~
¿ïW?íUÙP?î>3Æà¿ãí^½¥'v¿á*Vµï:¶¿àç'Áåèþ¿íõ¿4]ÖUNASNone?¼ûí`Ìm?³R´´M¨'?–uÚÏÑ'é?œ¹›@%³?ë¬Ó‡•]3?µÿ4q"aÙ?ÇæAÄËL…?×'BØ?›|2cBC?«ŠŠfî· ?é.­:Í?Ħ®¼9)¤?ɯ·Öq?¥'bK¥Y?´™l±7»?š+ òH8Ø?çH$£#m?¨Ë8=
î?¿í÷:Ýò?£/À)‡QÕ?"U³æžé?†¼õšxß?ëg""ñoK?¤'ibÖØ®4FGL J1735.2-1640¿ïDF^ç @ ú_"ÊÕ|À:*M)~~‹À;ÏžÙt{@4¶Ë®"¨@ÔbÞ©ª?Äü"_öŠ¶?À'KÊ-á?ùôàM/^@½Ï®Ôi?°4íóc?ï-*ÛuÝ¿ãj'ñ¶'!¿äM'àAô—¿íh!Äuæ?ЧÍęw‹UNASNone?ѐŸ0›wö?¼«RŸiÕ|?µ	"Œßù¬?°=ƂjÓ?ä–}ÖDÏ?ÁZÝõÜÉ7?år"i‰:?ɽ[ÐèÙ?À'ŠJ¼}?¢½©\  "?Ó?³HUÃ?Èç­ðA"?áòåÝÀm?°ÚqÍVÃ?µo{«?˜ØßKϺB?Ö¾p¥¹¡:?®áêòƒ,
?æ%`9ÈEœ?©9Ñ-WZú?«MhÚ?'¸`/ó'?ÐSuëg¯?§¹qâ0 4FGL J1735.3-0717?Â'¢xåÅ@*":귙_À9iݞ¬(À;l`Nq@2pÃa"@	ÿ&ò³?Á0/GÁ4¾?Ð0&£Ø·½@»)'<†@¼ƒ †]R?ïÞM}·:ê¿ßøQ{¿ä¥žŠš"V¿é+î›S­ý¿ãœ/vQ¿ïö¢¾ÜIBUNASNone?ؚ
¹Of?ö ^9l?Ðámy‰?¾ÔÍÁÁh?×Tل'‹?ÃéŸ(˺?ј:¬ìó­?Éý^zÀ"v?Þ¬ÀÙñœr?ϒ¶•GšÂ?ÏvòBßÂ?Å<^ë>¤µ?Ùð*ÄÝ#?²Cn#%œ?Ä΂ïŒ9æ?¦:óSK?Û¨"Ã\¿|?°}2«Ö®ô?À³Z	)«?šsÄùËH»?Ö[ûƒç]-?´äX+'?à¥+»Ëþ?³;eçn|M4FGL J1736.1-3422¿è¼wÑ·‡¿ò¦J'ÛÀ8ϙ O–@À:ùÞØh'@üpí(@ÐÔ¦2.?¾ÝþMxX×?ߙrb+Š@:Zà÷&=?ÿ=«‰Ü[?ç¹`>.8ø¿áþÐW›È¿Ð•ŽÝ}ôø¿ââ7ùk'¿îõ"€-¿ïø¾nèìUNASNone?}ÃäIᚿ?'YŽÝXI?ë$x?»ÖnÚRKv?ÃŒ± ÝL?»ǺGx÷?Š«¡¯þtÝ?"¬ŽÊÛ6?à+u'º.!?ÌÌ	î@,?ÞÓ¸£°?Ìn¨´¬ +?˜Z!Æó¢5?…û™@™ke?é¬À?bò?­ƒ–IϓÀ?ÆAºÊÓÿò?ªâY›¦O¾?}ìö©–?c#$Jg¡Ì?ÙF@=Y	û?¹Qôï­Xÿ?ã!Çf(ô?¹jHád‰4FGL J1736.3-2929?îY(2N0å?ö¹ïô8À9'7›wÀ+À:¢êºô]5@ç+¶'"Ø@FºÜà@G?ÎUíQy?׺¾A@
†ðÝMM'@1•@C'¿ïÿíUÙPi?ïÿ¾ÇPŒ
¿äXeAxEa¿æړ)=,¿î{J#9Àì¿ïÿèþ†®/UNASNone?È­É»ÜÐ}?¾^Ý܂?×S¬kˋ?ÈaU§Qk?ÜUn¶üÌ7?Èß
?èRÖ?¨ÀˆÎ*Ý?°ˆ
b)ám?А"ÁZÞ?Ë2»O¿)¶?æ6"õoã?ËðZèYw?¼Ë£¾.ñ?˜¹¬ÿïÝ?̕ۮ'N#?¬´T'í)O?åAœžfš?­Î{lÀ=?Ÿ%Ûæ;H?…7kDü¹?Çò¶TÊj?°‰¯å­ÑY?é
Ló8ó%?°¤8WYç4FGL J1737.1-2901?æa×ÈJ8?ø†jGœvÄÀ9Ž™‹VáÀ:b4¡È<D@«šêÒqQ@!dԕï?Ё^ú·@É?ÓÛÊ@«kÔ@¯d9Ö@
7_½ªÆ?ìó0®ôt²¿èmÝ¿è̞
²¿âZ£"Ôæw¿ï鲀ñ,(¿çKù"k9àUNASNone?Çé›rld?»—¿Z¹?¼@üD>þP?¹‰FËò?ç•æ›…?Å#BGB¤%?²"¨£—e?°¸ÚT»¥m?¿åW̏gé?Ào\°H?é³p±Y ?ÂpCå¤-?ÄÃÇ«ÓÞ?¢ÄÂdâóÊ?ÇÈï&Ÿá%?¨ß÷øâ?äÜÿDm¾?­ßAðíïA?˜ôÂ=÷^?v(Tç(?±b
™I9y?}ªü>S?í®¦Äé?Ÿem¡:ü™4FGL J1737.2-2808?¦²Dó–?ÿÉåA7Ø´À96"S.{>À:Ž"%¼R@сd®M@ßdš?ÏËø&êþ?ÁB%©Ý´|?øXà66ò@²°ÈŠGí?ç
«NÍÃm?Ú#‰<TD%¿ì¼W3Ã{ë¿â¥¥@–É¿çÞÉ^®64¿ïÿø="ßEUNASNone?ËV÷ö€µs?ÀS@b—B?°c6P¢Ì?®Sr'A&­?çÛ8]þJ?â]ìÇ<"?ÊÝoù$z*?ÁèAR¦?²?ºœ²ÁW7?½ÛF»2ŒÛ?åôðk^¶Ž?Æv™N?ë?Ï.‹¨g?ª-'td?·2ˆ¦‰Y?™SäîÌÉA?åN)ÈDØ?«§íjß?¼¢TЋ-\?ž¡˜5Òïé?§ÍÑj‹ô?' |âôÉ?êîØOEéõ?¡N68*4FGL J1737.2-2421¿ï¨pŒ°@
F:À9Ê/¿á+ÿÀ;|ùOâ–@ |}Šsï@èËùh6J?ÀËCòž¿¢Üü@q¤?æüC͇Þ@®r/QŠ?ïË:%•»¿¿ã¾>ê¡t¿ésòí†+¿çqÿÅG¿èVþ"p?Ôåè&Åf§UNASNone?ŎÊ{sý#?»{®&o«®?Þé~Âd?"¡¾÷ê?êV,ðœ?¼˜È	Ñ?ÒB¥¨üB?ÄÝJفîµ?ßaDBK?¨À_O+Ò?åï²#±_Í?ÅP8ÒêxÓ?Òl£²ñ?®aâÆ9ÆÇ?®Ÿ¨Tq?3ƒˆÆH?äà§3¡¨ø?®!‰¥-W?ĤJ]·B?¨ ¬[99?Ž˜}qÒ5?'°d"?ê6»rÊæ?¨÷kc' `4FGL J1737.3-5300?æNQû±wîÀ&`'ÏR¹
À:–n6>€nÀ<)RáP@Š¿â@inù²Þå?íÐȯܧ¿‹‡¨3
ñ?É–¾ÈÓ@œÄq^'?ä «†+(¿Ú§a£‰¤¿ä€ƒSld¿ã#ý5Je¿æ"!Í°!›¿ØûsT‹sUNASNone?ä¦!)˜?ÃÀg€6´4?"¯Õ¡dô&?xþ1"šˆ?Ö?·0?ÔÀ…¥o\?ë]·3B°?ÁQzT(?X¼W`S'{?e«¥&Ÿ,!?ÂWª"77?ÁqÑwÍ?é_®K$R?¬ïAs?•™'ó,Äå?}Å_2¨¯?ÈÿOmÖ?ªà˜Lêt¬?ìQ£þ ?"|Õ÷!t*?zõãRœ¼?eÜÒ$KÚO?»ÃÚ]Õ ?"R˜n,¦94FGL J1737.3-3332¿ïãÁl,µ¿íã¨TáÚÀ8àòFÀ:vIë	Ï@¯'º@K•"d~?Åúq¶%Á[?Ú7ÖÛïTŒ@—›ý÷è@¨0‰à"ÿ?îØn¡Hdž¿Ù¾(Õ!°¿á¨ª®"Ó¿ës³‹³'	¿éFõŸ<q¿ïô™=SHUNASNone
?–­ð=um?'¾'È+?µyà§Æ‡–?²ŽÅ¸<´©?ì›[‹…Ca?µ<vYj?¦}מQ½ü?¤Hèª2?³•jEkº"?°s
|rš?ì%u=mlÛ?²ˆŽBçg?´Êçuî@®?"˜´h%†	?ÂÀ,9r"€? èÿ¶<q?趘å"
?¤†ÜÂQ*î?†ÛìÒÒ¨j?q
¼?ÁU·‡©/?¤NZ¦B¯™?ëOIÞÒË?¤½´ßÍøu4FGL J1737.6-2350¿ï	^½>~@ÃNü½UaÀ9³ç't1*À;S~3Æ@m]–^%Ð@N€F}?ƾ—jjW?ÐÉD'@	ž³íQ@Ku&r°w¿æÞKòK?ïäÍ_ê2¿æ;À½Iø¿ä­Çüƒt¿ê2QáÊ	ú¿è
GŸUNASNone?ÙY"É‹î?¶™ŽëgG…?Æ>¤Ë˜'?½¯eŎ'‹?å•ñš¶á?ÂÓGîí†j?ÑT8fO'}?Ä%¾
ç©ò?Å>tez™…?À¨Ç¢8?âF³yÅà?Æ [aµLû?Ѕ}ª¡?®‰"Ôw&b?Âʔ$˜Ð?¢Üâe©Xp?ã
œk
ö¨?®ôWÛF‹å?ԃqkŠ,Ã?©ëð…y‹?¿^*ªš? ;ú -S?á҅äå–\?¬Œ°_4FGL J1738.1-2453¿êÅu™Îâk@U.€F}À9&ÏEM+À;"£Ð_@)Ö=8ñ@.v»H@?Äx"%çEI?昚ËÈÀÏ@4‰¾ZCB@(ç-÷	?ïñýwŠ%?㲟YÌúð¿äpYߚYÞ¿ìÊXÿ°J¿ìb2Yï_Ÿ¿ê"tÔ¾2ÖUNASNone?†¥Úb°ýŽ?ƒ×Pš,4í?é<q
fŠT?ðÑé?É£Þ0:Æ×?¡³ðyÒK?›W4¼[Ið?¨­•Ðêp?æøŒ9dN?Ëmºå?òÀ?ÐYtAq®D?ÉcuÍ…?¶p.ÔãÞö?™Æñ¬ÿ5?ÞLùÝÎÊì?µˆ­'ö×?Üúlø=X?³qì[÷
ë?zi
…è?f¦ƒ!JÕ?éV}Ehyò?±O.®âF?ÉÒ–5'U?°¡¾AIáÿ4FGL J1738.8-3241¿à)֘}Î¿ç–Äg£}HÀ8ð"¿?EÀ:'o¶q@µ@uU«ÿ"@ZÊA¤æ?Ƒ®éŒöô?Õí3	AÈ!@	]®f°8B?ï‡îÁ"4€¿ïŊîÛëN?ïùvÿ:Þ"¿×¸o}f],¿ébü¹úb1¿ì¿Í_ï©Ç¿Çè5žrqbUNASNone?§½ "ç<A?·ƒ—Ž'Á?µI°šV9?´ù ¤Æ?ëÚ÷÷>Au?À'ÏLÖ? ¼ÜEå¬? YÍk
8?É!4E?£QΩh`?è¯iה"þ?ÂmhÌEõ5?µªû[À܍?'G
ˆ‰o?ÆëGPß?¥Çí«0?çÎÀP$o?¨7dÙ(h¼?Œ…M7<"?wdcÜòjÒ?Ì Øÿã?´ûì/:'?è…Ä@Åã?µ¯¸n9:Æ4FGL J1739.1-1059¿Þe¦'¾r±@%7â–é¼À9êuWšñˆÀ;r0˜N?ÿ@s¸7ê@P¸d_ûé?ØÐ\Ä|Y?á¸é‹It¾@7褙§Ü?ý¾îUÄE?ïþèÞ{Jú¿åöŸcÝõê¿â^þ]hã¿éùøuȿ뵃Úët¿äHŒ`ÌUNASNone?ͯäf­E?¾¾Ý•äÂ?Ç»uy_²?ÀU¾"î"o?â¥Z¨Žh,?Äþÿ\a?ÒCBÃê¤K?Î'pn{?Ùi0÷v.Ü?Ð5"™2?ÔSŒDŸ,Ù?ɖ}J¤ã?Ó`IÍe£?ªÙºX ªø?È.H¢@Û?¨ÏvéÌê¨?àDV$ž<?­Œì—˜t?¯vҊK¯9?'5€JòÜ£?Ñ?ÈtdÖ?»aßС¬?åis!¡?»?!T24FGL J1739.2-2717?éPx`;K@n½ÚÁ'À9UçòÛÀ:¿Véá@Y×p"½'@¶Iû̔™?ɟSÂÊÀX?×%àº?@Õ"~°	?öãXAµ'?ïGˆÒy¿å¥ƒb¯É¿á¡—)|Ñ¿è[@*<•¿é\žÊù¿ïÿÕ"[ʁUNASNone2FGL J1739.6-2726?¬Áó"Úˆª?¡Lɔ²~S?ɐÅÒ;?½¬É¶'?çî<•=Ñç?À(ÏXǛ?¦=›¬
?©ãJ"1¬:?ÄÊÏ5`ê?Âㆅ_'?é•3'rT?Ã\±˜ Փ?¿ÑnÁ¡X?œ_Ÿ¶Ê¢?Äô:I
¦?¤ÍS
˜'­?æÒ÷Kˆl?©öèt{?ƒ"Dˆ"a?jù7ÖÝr?Çõ7'*?§ù¶çÞ?é´dþñS1?¨ky½¯Ä4FGL J1739.3-2531¿á÷'ë#ÇR@ÖûÅÜmÀ9ÚÖzËxÀ:ÉŇ^.@`æzGð@R):‹í	?ÀÄq‰…$m?ֈ$;ɄÄ@©(¿;ê'@‡rÑÙ¦û?ï÷º· "¿Þ}nàÞQ¯¿ã ³iNx3¿æ:½ …«¿íÍӒ¹«ˆ¿å¾Anµ?UNASNone?—ÀoPÔ(^?‡ü>$¤?á'd-Ã:¼?Æ*AÌË?Û_0¯lH?Åß«|1'?²SÜCB-=?±æ¦ŸœïL?Ôô%¯¢2?ÈÚr0'?ã;qŸÆ¡?Ƚ*ŸÂØ?´ÖIïr‡?•2½Cq:/?Úm'Nb?µáMfoҕ?àHÄ2›þ?´…¿US?˜ð:Dą"?tI™?§?ÇX΋$;¤?§0£æÜ?ébJ‹Ìê?¨›]é2Å"4FGL J1739.5-2929?è²À=¦	?ëÌ¢q¯À9{'±HÀ;MøԒ"ì@5#ä`½/@$Þ˜¯?Ғ(ÁÀ)P?ïûB+ºü@úô­¼fM@«À›<8¿ïÿù³>†?ïÿ~'Ø	?´ÊÅ㤀¿ì51ÛD^Õ¿é8›‡°c
¿ïÿ+#š8üUNASNone	?¥ˆˆçUÉ?¢4f&¾ty?ÞÆt°kÌ?Ί+@ˆ?ވŠ^ß©{?Î$ÞPms3?"Y]ì—¤?¡¢E= P­?ã'W‹ÙK?ϋÂ+?אrÛq?Î˗Lǖ²?Á)ióµ´¢? £+:Ym+?Ґ¿ÓãX=?±m!›WAW?âmE™ æ¸?±ýU¯pÁ?ƒ–÷vÊg?uÈB@>?ê¹,f‹¨?³¿Gå©á?ÃáàVù*ð?³£*³¿á4FGL J1739.7-2836?»Eõÿ1_/?ôW½;_QŸÀ9Ë
F9 À;ºB¿˜0ä@ W·¡íP@i¾N"È?Òë=%Op?ïü ¨Â@(¸®1×?ý%@œ'hz¿ï÷&b?eF?ïölmçd(¿×Xï»^h¿Ø•o¾Sã,¿ïâa9Ö»?âN¦±\UNASNone	?›âé±/á?—ÁÿPæ*?än$ÛÇXš?ʉ=éÔ¡Û?Õe‡¸f;Í?ÉÚüƒX{?œ¹q,M? »*ts'n?èwb†™Ô?ÊãrP*GJ?Ì'òãî…î?Éã\fîoZ?Äøn·yš?£A‰5ª¼l?Ùݎ|G`þ?´Wû²?ÜuL\â5?±¦{KÓo?‡@-$w?€ot¿*sr?ì¯bѝf?°¬CŠ?·¤pØ;?­±Ÿ'ÏA»4FGL J1740.1-1928?Û-'«äu@Œ¢:RÀ9E,Ñb¨À;ÀJÞJ¤@×ï½èƒb@#é Àiè?Ê©œ)&??ϲ?WÙ±@§~"ƒÖ@Árážëé?ïD8>4ï¿ãu]ÐÖ¿êøÛH"¿åŒ){D¿ïÿ>¤€}i¿ˆ5ø=œòUNASNone?à)qß¿Ý?Ä]&Ž?ÄðrÓ[Eó?½jC²Gâ?Õ4äv'ÝL?çýµÎEe?Çßìø
'm?Àd«;¼›?Ð<'Bz@l?Å,\èŸ?áéñ À?/?ƍÌò¾Š–?Òä~ç«	ï?¬+ÅØqK?ïÀL£Í?¥}O¶zÿ?á¡Ðy´–?®è©øìMD?Ç$à2"
?¡Y `M¯?Ê4îÞnÄ1?©ÍÎôÊç?㩌;Ãíò?ªx2ýyTS4FGL J1740.4-2850?ÌËÊ
ƒD?ð
Ð"¢§À9†ñ·û"À:s¯þ_ìÐ@"ù‰@? §??Չüm¤HI?ØÈáè@
'h	ԕ@{……e…¿ïÿ2Döª?ïùÍKw͗¿ÚCC ¼
7¿â˜ÜP'`¿èÔ6¸ù±1¿ïûgêÊä•UNASNone?µ Øf±5?°V<<€?«ËʈPuÝ?­#<–•æ?ëŸ(U"{?¸t|'šo?¾SMÅ@N?¼ûé¹Ü²6?±Ý÷éM.?¹ñéf=î?éùä(`Q?ÃbnI±7?ÌدÕ}«?ª%ÃB¬Ë?ÄnÌue¨?¦ÖˍÕ.?ãÂøW¢G+?°^ë@ß?´è»'D€?¢ÃMö?
•œ¤Ké?€ÑùÉgz?ìî¾9DÞÐ?¤õKÍ¿€³4FGL J1740.6-3430¿îy3òàÀ5ĊÞìÀ9ùóEÀ:Í£ùZÊ@‰éOdl;@‰â¢!'˜?ÅÐ2²Ú³??Éédµy@ÿEÅÜï?ÿEù ½º¶?­ÇN¿èpöa7¿çBYì°¿äö¦_¥¬ø¿êõñ‰D·À¿ãĸ;SéUNASNone?¦¹oFô"?™³õ8,à?±3› ƒ?¨£F¸˜e?ìb·e+,¦?°ڊÙ?¹DÓÚFŸö?´ÍlÑ;§Å?©ÍÜÅàÀa?ªʋ^ê?ë:‡¸Yü?¸Վ…vÎ?ÂQGúü]ò?¡CÁšR?¿a—ÀËÉ6? MV×X4?ç{	'o]?¦';'ÅãP?¤sDL>??‡æ±ª×WÖ?´æ³Š°ã?–ë}Ñ6á?ì(ŽäÊÈ`?š	қ™'C4FGL J1740.7-6750?²|>NÀ2¯Ë':)ÇÀ:ƒž…'À<&c{Ð[@ÑA}£ÄÁ@°ÚB×%?ÂVûºKü?Ï¡Îò@úœ@"0{ÈÎ;@Všó
ú?ïý«&‰×…¿äØڌ¨ðO¿ì{¯¾Ÿ ¿åЭÍ-DÝ¿îDý[5¿ïÿߞ¶ŽóUNASNone3FGL J1740.8-6755?ëí$ è™?·~*^h?´/˜sÖó,?³N²?¨Î…)?£Ò¸ª‹—?æò—Ì(¦2?Æ:êµÆøY?Äh¶cyK ?ÃT¸8¨?¿™Ô×È7/?µAª=]"¤?ç	ÅE¼?­½?­sK?º´Tˆ«Û?¢Ž­»{r?Ɓƒx•`¢?¤4›w»
\?äɍäâ¸?­ºôš&?Ëíµ)Áh?­•3¦o¸?ÀìFy³´?›Á߆Š²4FGL J1740.7-2640?Ë:Ý
Y&Y@ÕinX£/À9¨‰ò\©NÀ;L'݃Ô@ð¿Îâ{¶@;½Ep?Ñú"å$²g?å7]ú14@‰0«½?þûþ0Gœ?ï«íßl¿⎧Þ*î¿Ø ­ŸŠõ<¿æŠw½¦¿¿ïÑdBSb¿ïäó¿ÕÃkUNASNone3FGL J1740.5-2642?—vÓ&Ê4?œ
*$a?ŌÖ8î?¿$ôB¾Ä¶?éá؎(Ù?À")^Œ?¢·<s¨÷~?«SW£ÿ,ª?Òͦ‹Lsß?Êñrý&?åm¸ó6™?˯#L?´çe·þÄü?'VɄ¸Ì_?Ød}'öRš?´Ô•68ÔÎ?á0ԇ"þ?´n6f­ø!?"ʇ{›O?v©:¢fío?Ó#k'Ë?³¢wk…hB?åÐ6í\¢?³§ÃÃ1ʇ4FGL J1740.8-1832¿ÛôW;ŒYP@kÓ^·E|À9ÌY…­S‹À;G¼PíX@´\®T@ƒ¦Mà?ÌûWϟ»?Ìs¾ÿÖ¤@öU&£ø@Dz"ø?í]ì_9K{¿Ó¥Üû(¿ã²°â
¡š¿éòÂ?U*¿ìÏ÷>^‡¿ïØÎÎ.̜UNASNone?΁\CÚ;?¾I"øºN?›FH,Üg?–CÙx0[?ç…vºˆ&9?¿sšZ‹?Ñ_Q7EƒÃ?ÁC Ѹ×?´©y•~$?².iö›F?ä»(1¼ÎZ?Á³«)¢2?ܟoë>Ø?´'<ëë?·5CètS¼?›8¿X§8³?ݓ™•÷¬9?²#æ¸ÈÕ{?ӆ‰›má?¥¤¥	TãC?µsŸ¶IZÃ?˜sÀ䜥?ãŽG;€H¶?¦o·21Ú­4FGL J1741.1-3328¿éšp²Ö½£¿ù]ÄuqÀ9ÞL¸ÒDÀ;;3$º¼@§T ¾'v@$ÖÿU¶?ъ'¥aMù?âjd!èˆ@.;|­Ñ@ÍLVšÁb?Ü3ÿ`óµÅ¿Ì-ü}¦ü¿âԃ ±¿àIÓpóˆ¿ïÿý¡UûŠ?ïV⚔k\UNASNone?²åt[VÊ8?«_JÜh'?Í%`Sã?Â>ÑG_á0?æYùnµQÁ?ÃQ$²É×?»:[*|?¸ÆݝCœ?±4‰Øó»1?³k†®Ë©¢?êr#_Ù?¾Ÿdú\ƒ?ÄÚ1µáPª?¤S@"#¨?ÍU cE:å?«ªyc]1û?ãt+y¶]?®¨tú[?¶2Ì	»|È?'ŽA-2?Á)ìF¨?«rª©7ñ3?èï+mB}?¯â2E j;4FGL J1741.3-3357¿îÿ–ú­Ü¿ýÔlƒ¶ÙFÀ9Ä«^½ûyÀ:Ñ¢¡€è@ ¼Ü¥1þ@ø¼þ#@B–³5L?ãõ@‰]@ƒm¨z-@ã·­Uä
?ãÔ<ÞÓj¿îÿð:»?íD8>4ï¿ç.þúG¿ïóZ _†x?ïIÃ}˜²UNASNone?Ù55ٔ?ÌeRýr‡y?Ü36³¤±?ÐQH`®b"?Åw)r千?ļKé«q?ǖØ¿ã#?Ï["Ž›ÀÐ?¹Ò-ðQ¦?Çñ)W3ü?æßùÒÑý?ÑK}ëJ,è?ÍJ"±Í?ªa°ö®–?ÊÐ5ºT[?ª[øÐìÉI?áùZ©ä÷¥?°Š:?ß(`ÛJš?؈Å(œ¤?'a<=x4?·>ÆH?ßÑÃÖ Ýâ?؈û¿M.4FGL J1741.5-2344¿æ8?tè'Ú@òÒ»#WÀ9Ê:̄¨qÀ;´w K@3Æ̈́W¾@NˆÄ_@?ÑcáPè?Ý°Dä6@
Ž6A?û.'Å?ß?ÆßÅDd«?áÜlýÚ5ì¿ß±ÔÄ(¿ê[Ы~žl¿ï$ìH"É?ҟ.Äcœ²UNASNone	?ŠGßDùÔ?'ž¢ $L?²¶¸¹=c?®ˆH%ã¼W?íT)«Ôñ?°(6ƾ?Àˆ!¡ì"€?¼Þžÿ€e?Ó¤½åe¬?ʐý%8—?☤ö¨
?Ét^§¡:?¼ËՏJº?•™"2Ÿ"?ÈaT‰Eø?§?ùª<Ï?æ_ìøôj‹?«¡6‹LrÅ?¯.0ækŽî?'ýÍñú?È'm€®…š?«ü×èÔ+?èA'm¥«?°ÍÁ–4FGL J1741.6-3917e?Û`6Oâ[ÀÞÉâ6Á]À6ücÔÀ:cã6îª@~ÇäیX@cyú—á3?˜2™sW;?‹Ë<Sî>·?òV¦4²4@ySÙFí?í¬œuìì'¿Ò¾ku™à¿áÁŸÂ¨†œ¿âCn9œ¿ä;˽Ù¿ÐiÕOçŸUNASNone3FGL J1748.5-3912?µ¢ÄB˒È?¼Õ@EyÈ?†ª•"Q˜?"lùSM?ìðý#,`?À-T5÷½?Ú1©ˆ:'#?ÏÛbXґû?±±]Q*ÔH?¿¦ß˜+G?à°ÿ'½\å?ς7'_z#?Áª¶ï:?¥«œ›‡J?©â¢À‰9?'óØPN»º?ê ë&;Ì?§ž"Ê?Ґµn¨?»%mÞO»#?Á.H9¼»Á?±—=U.ßl?âlb™¼?¾ùC«[ÿñ4FGL J1741.6-2730?çIŠL
Žx?÷âCV–åŠÀ9"uÝÒ®ŽÀ:ys›Ùú@ìØwÐÇ@Z5Ö|?Ë[›\<kì?ÚÓPtŒ™×@zÄÂ<P?éB‹êÂk¿ïÿÙÐs?ïÿÅè¬ý$¿æþýÝ;¿ëTGÛ`ä¿ìŽyP¨9¿ïÿgßbP­UNASNone?É4¼Ô¿0?Ì»ç•0Ã?ÅÓô¾ŒÑ{?ÅKk(+?ä=ӛTÛÕ?ÐWÏ@x*D?™¼þ³M*#?§.)Ÿ?ر§iÁÜ?Ð'lB?âÙDŠ0µÁ?ÏÄjLû¯?»T'Åã?˜|WwñÆ?ÉS%¾î:?§Œ»ƒ–¤­?æH³¦L˵?©oíå[ào?s+F¿-?^Ö5ê¥Äs?ؤڬi:?·óá"âæÏ?ãՅ<M?·û0¦D4FGL J1742.0-3020?îòÞúvÔ¿±ƒÙÓ-©À8de+ÓÃÀ9 çJ&"¿@¤_ݶ)@ùGÏ¢j#?åãM"M2?Ò'5ø	'@ĸF-
û?þ FnÏ@š?éñUbˆ
{¿ÕAuÁ"I¬¿è±ÿ÷œ"0¿çù΍—,Ø¿ê«-u"›¿Ò¸`Jã(UNASNone?"ã©/d͞?£¾<G‹µœ?¡ˆ±¹]X?­5Ìì],?îHWšôƒ¾?³aèÕÛò?¨ü—™È8´?«ç¤©7?³†&…€ÑK?µK‡Dþ/?ëÿqµ³bL?¸"Ž$:±´?¶RŸyș­?"T'&˜¤?Å`ì|XÚã?«GŒÿœ?çÝpñ°¶?­‹¤Dóƒ(?'D«V$g3?sx^Q¢??Š7CèAªY?ª?©à?ïNCgº?'á¾ÙÀº4FGL J1742.5-2833¿Ð!¢ä¾Rƒ?èÃoõPÀ8Â.jÑÀ:"P\8æ@i.r.E¹@(¤~Ïé¸?É@h:{üÑ?Õã*Ý#\&@qìb"IÏ?údDÊ=Ñ?é"L["e†¿Üaq¦3[¿ãONâ'/=¿èÄ1Bm7ç¿ï;_A"Û?ÑÂìúUNASNone?€=‹¤÷P?}ódË~›?ºÌÐðCmA?½
·Ä?ìeo³cµ?¾nÛͼìw?—ûPxHN?ŸWÏ߯s?·¤©45á?¶Fîb&¦?ì_Ðç6Ô?·6uÖŽ?±T#a:5Š?Œ27à.¸?Åݘԯ}?¥Zø$öÿ?è^^¬óo?§¢ÑDió?f>–Ó©ÏÜ?TÌËÌ-º?¸¾¶ýLÜd?Ÿô‹æˆ?ìÑꉂº¤? @Íÿ:4FGL J1742.8-2246?ÌÔv?Þx'@
ñqýs]ÆÀ9°(¼·«ÓÀ;"bGóµ@Š•{&çË@;'÷
è÷?Ðl8¢Þ¼¹?ÛþÍzò@Ã#·;k@G91úÎé?ì«ÊÅ㤿á˜Tà'^¿â[óEÝYã¿ê*€Â2?¿îfd¸ç<»¿ï¸àâ"UNASNone?ˆQzƒ%Ù ?|^E͒Â?³æÑ)š¤Ñ?­|5ãˆÙ?í!ßðÀ?®Õf×j?Ú¤RläÅ?¼æïÃÛ{?Åz¦ºÒ}¢?Àº†þÜ?庭<°'f?ÂôÃȆ…Ä?ÁN¢7½É?žÚÍå×U?Çí©³O¦?§}_̈Â?å±:-<¤?¬Ð°§ö+?±{S3>$?"ß®ÑQë)?¶ËÜÄxS#?›"Ñ×9_?ê÷	1
?£[LÀ•û£4FGL J1743.0-3201?ßfÈäi.¿òlÛzåylÀ8òñÝ'ŽÀ:i›€#¦Î@;MÄ®ñ@e|áÒîO?ÎÔ6SÏ
?Ñ!Œ!‹ëÜ@2€l'Ð@¤æ'™ð׿ïèùôMDV?ï,™†Nc:¿å!"dƒã¿æ1Iï7Zà¿ç~Ê-ëÌ¿ïÿþøþ"UNASNone?ƌ¡'Sé–?»6úá‡Ì±?°G0Ϝaw?«KËaÉ
¥?èSñœ7ym?À†¶É×~U?¬'Ô™ª¦‡?©€Ý*å¢Ï?¾œ{"
¦?½",BÐӘ?êcSUróâ?¿x3yyS?¼2Mðíèž?ž
•N?Ã)ÿ¢×¡??¤q©6¥-?ç¯6Y,Zœ?©$ ÿ·1?§têIœ ´?j­wE¯Š?µRM¥?žy.oé?ëè'Ä5??¡÷ˆÐK4FGL J1743.1-3049c?ïùÃy֟x¿á"<5:tpÀ8®XŸÔF>À9ô"Ÿ^Õx@—'Ýè¨ö@@Ëò¤Î?ÊÈË5rþz?Лüà»Â@éý_;Ð@Ðyí¬Á?¿ïÒü›K ?ï½pŸM8¿çh*á«I¿ã'™îLÏ¿èõ¿¿óö\¿ïü\§ ÃZUNASNone1?²îÜ@ú‡?¸'4íš—?¯é|]s?¯t)mÌî?룔p©F?¾Vg|eË!?­+?´Å?°XñjiA"?ÃkrrË9Ç?ÄKQrƒ€?éRsK96B?Äóù¡¶c{?º`—÷J-?œÚ ·L/¥?čŠ;02%?¥Å®=š=Ù?琊rSê1?¨á}4Ee?šc—Éiœö?‰KºÎp{?®°›óã?œ7S7åi?íL¸8³Ù?¡ˆ¸ó¦S4FGL J1743.4-3123?ì_&óû:¿ëú¾ï>'À8â֕£jÔÀ:@±NÂó@ 4^lFû@Ú½]Äu?ñ)ŸÖÊ|?ÎÕ< ˜@D¿ÒéF€@ßÿtißB¿×ù\B 6?ãsʒ`¿æ^B.ù"¿å#•0~M
¿ä{õO¡S¿ìä"CÆÿ-UNASNone?£³Ð"§+? 3Ó î?»eÆN~'š?Á¦‹{¥?ëX
5çãZ?ÂÙi1XN?¸b!Å>ê`?½ëÑ*0÷ä?´+Ã{KÌ÷?¾¯ñ%¬hê?ênCWî©?Ã0ÁE"?¿²'*Í»?¡eëÇáø?äÁ¬$Ü?ªêN]2ù?ç(ĪT=?¯CO،£$?¿¡'ŒùP'?²úXY¢Ÿz?~–ªe:?ôÙ·<,?ëϨ'A1?³{Q= 04FGL J1743.4-3406¿î_pö.½ÀlZßI§À:ZKÄ#°ßÀ;®
9>åï@áÑcµ\@Â=&Ñü?Øéq}ñg?ãÜ|m8è@y‡Æ2~Ø?óï•!îZ¿è$EÅ.î?ãü`£®ÆR¿Ï|èˆêö¿åÍ´Þïd&¿êŸÐJ/Îû¿å¾§°³'UNASNone?£¼Ûò?›hÛ
VVa?Þ5ÑnkÃ?Êl¥Z‹s
?ßhö>¼?Éåž1ù´i?«t<®mpu?®Àñfì?Á§y"¸º?ÁýáMw?éÞÝÓõ:Ë?Á9Šü…2Å?Ë6
'ù?¥ŸœûǕ?ÑTæÄ)?¯n'E¬jÍ?à§Rçß©ß?¯*"&Æ?¾?›o·žŸÆ?™±à%Ïc?ØÚ>±âu?À°M¤Ù9?â·bêÇH?ÀIŸçï¯4FGL J1743.4-2406¿çÛyoÏé@yߖÓìÀ9¢"'¡WÔÀ:èñ«©f–@ê£q^¼ú@Aë¾íç?Ê{‰¹&Ò¨?Ïe7ýO1@EÇ
âA?ÿNç àö%?íQŸ?ûs¿çzä7Lh¿èZ<ŒxHç¿à"à4ˆÉ¿ïÿþøþ"?ã8}àU•´UNASNone?Î&gtð–?½¬þv
öÆ?·ÎáÚ}!?±êÛ~ޘ?å|‰ð't6?ÁŸãD•²ñ?Ð)Z¿OI?ÇöÙ£Ù)Ú?¿ÞçÇo!ª?À»?§_?ãïu÷²t&?Éè<¦½á^?ÎÄOQµî?¨{•Ð½ut?Í@üA?¥éÝ4ˆ?ãk¨[S§¾?«ØÂ1LFÕ?´0z9Ðcú?¡"4€ºâ?¬•ÏŒ?š«Âú–"?ë° [Ôˆ?©æ~ÆAu^4FGL J1743.6-3341¿èåxÑ^=ÀÝ!ê6À9•$Š#À;‰¾ZCB@ m™Y_@õ~íEé?è&ûíKÈU?È/«©¼|s@øZðŸ@[2\sž]?ÁHç$'Ú³?ènæ4'¿Ëñ.Uþº0¿ä5çéóN¿ævñ~\ý1¿éIO4¹ÀUNASNone?©­!ùì¸×?¢ Ä¨ò?¢Èß´Œ'?¬*uÐÛHN?í8Ÿå‹©?²*|•†O6?ÈhÓ!fÄr?ÂÓ¥›R?'qçV?ž~Þ^vÐh?é]£,‰?ª'ÑxJÓ?ÐcåŒϬ?®Tu_¤ÏE?·›ù~-ל? ²[úí
?äڎ
/Ý7?®ØUé}S¶?Ó¥ea–?¹?%É­3{?ƒ:'Ø!y°?‹Dg|ßJ?åàc7"IO?¹œ/'v¥¬4FGL J1743.7-4321¿Ó2? ÝcQÀª#žj¹²À9ËÍiª¾…À;òHv'VÕ@äÖÈN7ñ@^½$¹?Á–I˜z_Ã?ádv6¾/@9ßÞè@Ž÷Õ:?豈bîпšàRe¨{_¿ÞƧCÑ;¿éûß¿˜±½¿ïցz"ð¿í¤{	‹™ýUNASNone?˜Ì™Yf1Æ?¡Td^S?çÖWò°ë–?ÂeGg¡yú?͍
‹o?ÁCú¯?¦ÅnAXd`?¨llxÓï%?ã-Âm^д?Ë	DåFQ£?ÖËÍ]R?Êf.P€?¯"ýÆ5V?•˜µv$ÈW?è>U	µM?®^Ë$'?ÇFܝu?©ý?5‰?¸cVޛ—ó?"oÑ«ø$?ãc~¾B9ª?°¬%%G ?Ó ,ËÔ¦°?¬™ØbŽ…4FGL J1743.8-3143?è#5½¦Œ¿ò:øúRAÀ9['IWbÀ: ¼X
ƒ@!]úŒÎ…	@Õ¼{`É?É2ØÅS†»?Ÿ!N%Ê6g?ße)ÛÃP@Uvꚿí!ñÂO›I¿ž-QûRú¬?è'_³Ä¾¿å'§¢pØ°¿è<Èk.L¿À•¸#®UNASNone?žwŸMY?–l÷æñ<?‡Eº_å?"Ü›wG¯?î²Ã,Ϋ¸? '9c$I?ÈÑãÜ~w?Åø×ÂÈFu?«¯Ž.{?š• 7?éŒ/ÀlÖ?ÅÿÄj6#?Áèp"Ío? Ñce4j?³–]½o¨.?šŽÙú¢áÙ?é#Ş?¤ö™•B´I?Çæà{SÎ?±§ä·Õ?†ÜU—ÝS†?"yUa>™?éâÔñµ¾?²>-!UË4FGL J1743.9-3539¿ã%—ԝ{¦À	¥%1À9Í:óñÔÄÀ;bʤÔ`?@1¡¸¡ó@‰ÂÁ±Ø?χ?ÏÏ?ä	pA0¡Þ@+vö×bR?ûç­ôDŠô¿ëÝâ¾ü˜?ï2«M÷¿éÂ!øù&¿é©yámm¿ïüpßFI¿è!8>µÈNUNASNone?̛ºèñø?¼…"?¿ç¾'­˜?·¯¥ä»ê?äܺP ?Â_†Æ?°2/1"b‡?²²ž—{Ý`?ÑÍ;œ•3š?És\ŸA½M?åK'ùâ?É+'¸YÈ?ÇEå¼Å"j?¤ÂéÀ/…ˆ?Ä3Gk¬‹q?¢ÚŠZÊp®?å!´µãx?¬¸2úPÃ?£e£Sš©f?ˆ@–,οŽ?ä/
7ÊÙî?²Œ({ZŽ©?Õ57%ööø?±|OœÕþä4FGL J1744.0-2504¿ïù§—šL-@ƒá†˜5À9BÍl.ýDÀ:¨ÙRîº@¦9kÜr@§"~§¥Ì?ÌÓ÷8†.X?Í>@,•à@²Å"Ùîô?ð±BøΊ?êÑr¹[¿ç¡ŒâÑñпèÉaÔ¿èç¤T¿¿éñþë-
$¿ðUNASNone3FGL J1744.5-2506?ÓsŠÝ­x,?ÃZ™£;­»?¶°ÙøÂ?²5¥ç­?ㅤuê+ª?Åvï›ÉXI?ºLì$²î?¼þ®(e?Å¿Î]?S	?ÆÇ ƒ••?çFnäç¡?ÈHþ'ùj»?Íï_Ñ?©Oøá¿?ÂáñħP…?£ÌÆ5¬Iï?ãË«šç›?¬Û7´ø?‰aüçð‰?t<uk]ÅG?·h50cÙ?Ÿ§T
õˆ¼?ì­u¦SÃ? §ÎmÅþÞ4FGL J1744.0-1311?æïÐ!ëã@ çqdÇ)öÀ9®ù–Ys9À;Tpš@(żãÊ@íqåöi~?À‡kŸ‹K?Ñ"ÌHBŽñ@PLýߔP@‹È>?ïÿº*2Ùq¿À¿1ÄPÉ¿àÖŸd´µ¿áê2¾™-c¿ëÃé.,c5¿ïÿŲýîUNASNone3FGL J1743.9-1310?¹|UùüJ?¯OÞwÕã?ÈuÃYsç%?½1"Q¡·?æÁŸžãÆ­?ÁOE8³°?ÆüH"
d?Á©ï1Ú?ӍÁRøJ?ÆsØÔíÉ?༦ú"#ƒ?ÈÏø|\çÆ?ΝdHø)Ù?«Õ#0X^Ð?Ô&é
ì?°]˜ªc	P?܋=Ϛà(?®âÝ©¸úô?Тe ox?¦wlF?˅k¼©Q?¨ÇØh㔹?àÍr¨Ùª?²QÄ?c4FGL J1744.7-1557?ˆ>͔J@Ÿ§¨PÂÀ9ybA=·ñÀ;m§<ð@"ᷕƒ@ìC9+?½º›ÇÇ)u?ÏõðÝx@®@Îގ–0?übE1¸^×?ïÏXBaNz¿ÝqÍbHõg¿æ(Æ}}YG¿â£Å&p­¿íPA`ó`¿í±P$QïUNASNone3FGL J1744.8-1557?›…ï!Áƒá?'IßAe_p?ÍãÐ!Nåø?Âۆ|x?çªÜ~ž:c?Ã0ڈ)Î?¯]á'‰^`?¬ƒŠn–äG?Þ§§ŽÖ–ü?Çíçíýb?ÝlœL8=7?Çðjþþw?Ï®® @¦?¬¶^½ò¼?Ó7"™*çl?±\Yª?Üñl"øB?®t2ËX"?µÓ OSRò?F¥P?×»§ˆÄžw?­©'·ÙÎa?ág¸1³Ff?®f.JµÑ"4FGL J1744.9-3322¿ÚåN¢¿!ÀÎú¤vlÀ9x ]Øù+À;!ÖÜñ?@ES#há@Nc¥ÁÆ	?Æe
›º[0?ÝĄ^žò@ÞÔI˜Ð?þ§/ç¤>Ž?î&mó"¡ë¿äu°»õ4¿×Yӟпèi¢#¿ìpâ ôÈ¿ïôè_Op×UNASNone?†OeK#?wZíÞ?Ôí'À»SÈ?Âà™sY\O?å0)Û?Âò¨Êˆf?©CO˜Ì?¨à™ºÙ—?ÁûÁénÐX?¿êÓqo;'?éìßPª¿#?À²Z=ÿ?´¦fè¬(y?'ÒÍ`ú?Óuéî´S¢?³7ØƸù÷?ã°>+Q!?³VW™¨K?È?4Ñ?q7'yØ?Òÿ~¤Pò-?­Mîp÷•Q?æ	xÚ¶?­#ʂ'¥i4FGL J1744.9-2153?î#œ´£'ž@_j^B«vÀ9•
ÿÀ;o#¤I÷@0–¤Ç @DeÀN9I?ÐҋÿH?ϒ¤g"@í¶^Ì>2@GºÔ§¸¿ënM?ùÀ ?ëÑÇ]w)'¿âü¯þàÆ)¿èêÂKiŠÞ¿æa@AŽ•¯¿æžë/ŽcUNASNone?ʞ52F?º=CHäp?±7¹'‹b?©õ­'f§?ç1…Ê¡P"?¾øúB`Y=?Ç´;öô\?¾uÿ
p‹?ÅT²¦u_'?Á¨ºOÛ Ú?ä½ËÇdë?Ãý:ÉT½?È`»RW?¤ìàqcJ?Àp&6Ð?¡NØù¹Ì?åËÖôƒwi?«EC›¬U?Ï¡7cPĖ?¦	·rÐF?¹èŠ~Oa7?¤(–ùhˏ?äÚ ×aâ³?¬4A¦84FGL J1745.3+2338¿âëaÀíÏ@8~
"¾@BÀ:T3‹GÇ?À<*»êý9|@Mheïóî@`êžnëp?»
míq¼¿·&¨
u¤È?÷¸)W^Í?üàcR4ֿ°£?4É¿åmbÙéë¿ìŠtBrq¿å™Þ"Û¿è;?Á¶ï?âÊC…ÎUNASNone2FGL J1746.0+2316?íl¥Mä#'?°|ëV@ºE?£`ÚD? .1þíšf?¥ÔÐݹGÅ?«,^Ù\?íDÛ©–‹?µ¤™q‹V'?•ì¾Iÿ?¨êRØ2?°•g¶Ã¹(?ª­•™19l?ëû•2©y±? Kºœ7—û?™°˞½]?‹+Lf\?¹·N÷̃ ?šü†©&Ç?í4M$'1?P#Eø?"E+Ø;€/?…­êP©û ?±LK鬖p?˜ï(¾ n±4FGL J1745.5-2249?Þ÷t¡ù §@	šxš:À9ÙéðÀ:³m—³Œ@_#·SÊ@P:ÅΫÊ?Óµ^>J?à™ØZiÙ@	z™ÄaÄ@@d"µÔ㝿ï·]d_%*?ïñ"Á"g¿ëMa²¢¿ð?ïÿû-2h2¿ïí}±«´UNASNone3FGL J1744.7-2252?ç/$Ëß?ÈÿªB
üí?¶Ü]Î^?¹ÆDr|»J?ÇÕešEË?ÄÆ8:,x?Ôå"sé^s?Î:iD8êÀ?»ÿ?â^²¦?Å+a|¸~^?â
MÉ¿zr?ή0%¶[?Ì«vÈóu¼?¨¿KFcI?Í("¯b_ž?µvû,®é?ዡꊩ?´ÓšN¿°?Õx‡ž±+«?Åd*Ü%ãÿ?"Æ4§®_á?Ÿó÷ú?䝊‹i÷+?Å©' Ð{4FGL J1745.6-3626¿ÄŒÛŒ…TÀA&:ý,À9Y©mL3µÀ;KkÊSuÉ@}Š/™J¿@|­€k`?Ŧd׍?Òåí/Bä@…»¾‡¬?ÿ¡?¸§¦Î?ï¤Î(™Ò¿éšÌ¿¶¹»¿ã¥@@âÉ8¿ânøÁG]¿ï¡‰R#¹?ãJò|‰¾UNASNone?ŸÏG›Ýº?—_=ÅpÅ%?£ÉÓØçý? A¶V»Ê?íդ腒'?§hD½ŸâD?Ç1•Ž«Hº?佧?³32>mW?µŽ@^ïI?çÍ4T‡'ï?í˭Øb¬?ɧå–V?¦ò'&À?Ä|q"ƒO?¡(-Žrq?䐼ª5^?ª?#Vù'Ø?ÈÖ5Ikž?¦»%;Z=?Á@±(¶•;?¤)µ½¨?åzFo¿ÿÉ?®ÇÄ»4FGL J1745.6-3145?ë`U8ÒÀ"¿÷¨Ã ¢7À9·k;¸=À:׆¾Ë'J@‹øyMô«@Qw~¼ž?Í7•˜ƒ%?ÙjÈ˶L@7Lg"t@mºB±€?çÇ_¥'(¿á£tä®k¿â(Ùþc´¿å\ƒÄE>ο煇"Ý—ö¿ïÿÓà<k@UNASNone?¹3ƒÛ‹BÝ?ª"]¼fE?Èp7tÝ?¼ŠÁQáoÓ?æÙsv±'m?ÀUC[W´M?¶Nifª¤?°¡Ããíï¢?¬A_½çØ?¯:	ð«I?ëráNÍ?µý)OO»q?˜Ú`®`?  '"­&î?Âüø¾]¾¯?¢`žß–<?暋MPd»?¨gïd½¦{?©;¼ª>;?=v'˜xÌ?¸kçôÇš?œH»aaã?ë^Ç6¿,? ±%xfc4FGL J1745.8-3028e?ëŽÂiá4¿êÈè§æ›À6ŒŽž"Ô^À9¡PþU0@ lÒ³k§Ä@æJ>ès? kæ­ôo~?˜ëã=|?õ×??ñ/Q|I}?ïIše]R¿à
Õç'Áæ¿â#揲¿å$;´4ç¿âÀœ<âž¿ÝŽèÑQ­UNASNone3FGL J1745.1-3011?ŒŒ«ÒAn?›8ÿ$p¶W?sÁ1²¢²'?€ ^7PÚE?ïfJíQ¶a?Ž+juâ6?ŸŠí…D^˜?ªhQÑ^¶?ϬŸÃ¢@r?ÌRMvŒ"?瀢íLð?˧ƒJNô‰?µBª²$?œ
Š§ô¿?°NےÚçÝ?—Ö$‹T©?ëRœ8aì¿?¢­EGcP?'¿Â»fàu?w¿áw×df?ÄÁ$Ÿ)ã?´sH{ø?ꄷôªš?´;V‰Jf4FGL J1746.1-2541¿îŽÖOµþ]?ùMë­òíÀ91áìï'À:ö"o³í@n‰šs@1*å†×ö?г ž†~?Ñ!
Gé#@
MFðP?è
ۉº9³?ï±K(¿åV…í	¿åǐbcL¿ç§/^½O¬¿ë!¿îB¿ðUNASNone?ÛIb `}?ʶ"æ÷?Õ\ŸhDn"?ÉJÌ(rþ?δšj6aþ?ÄÔ¢‰?š¿?:ÛæÅ?¦í÷âÚÏ?¿Ç)o–_`?Ã]ú×Í?ë1 Ø6TÞ?Ãî
ïaœ?ý+.ÛýD?¢+Ýãäb?Èég+/äD?©LòÖ8§À?äÖ[i}Ÿ?­5©/âÂ?a=uÍÃ?N%¸´+ì³?Ã6ë"P¤?®•lj‡Æ?ë![ˆ¶	?®'|ѹb$4FGL J1746.5-2019?×ùG%û´Ž@._¢ýÆjÀ9l~|áœÀ:Ø¢xelk@µètž›@.ƒþý¡?ÒVñé¼Çœ?іé;ƒ)@	±ÕšÑ§þ@€¹xÝ?á7¢~D©}¿¿K¾ß8¿êTݧæcw¿å›ã@+¿!¿èSZ_òÙÒ¿æìa¢—oUNASNone?՜'q‡ß?Ây¶k€Û?È|ßW÷s?ÁÃ[RºEü?Þ%zMb|g?ÇÌNÜÊ?ƪÌúme?¾8æAB?ǚ­ÍHQ?Ã`ñ²ÃÌ0?än¡‹/P_?Ãùá)c-ë?Ó©Ü<?®áið'ó{?ÁŒsñæZ=?¦«|ey<?áÈYhf#?±Xçѕq?ÁR¥^¾?ž…×?µ…ꡘ"W? l•µLL¶?èú½Â‰Uå?¥ºÌF!¾4FGL J1747.0-3505¿ïΝöºKÀ³~²†fÀ9;AÖNVÀ:ð~gäì@¨ç ÐH@€"Ýz™ú?Òý¤Ûìû@?àž«QR+@3¡/?ÿ¸†^©X©?î̎^''·¿ÓrP¿á¿ã@Š3Ë	¿ë©Ùîm¿èˆ"#8m¿æ)7fžšŠUNASNone3FGL J1747.0-3506?°@?WŸÞµ?ª'YPâ
\?äYîÜhõ?ÉŤ…<n?Ó<qGèh?ÇçLô""ð?««] w4S?°¥c²mê>?ÓQ!»‰B/?ά…}Èÿ˜?䜹H3ë¤?ÍLš¼_®«?»m	åtrÃ?Ÿ¸`ƒEgß?Õè¹²7ã?±#®'´@ñ?ážêOÕµ?±'2"ÒK"?tÆM¯³›?`µ®4?Ù&Ûߊ‰­?¿è D?ãCtÛSô?¾û} "4FGL J1747.6+0324¿îü"J|ü@/{À6âëÀ9®Hn-ÛÀ;¶·»*ä@™Km¼›ý@Λ¤5Õ?½µnryo?Ê0¬O·x@
"­äª9$?ÿlyöf#K?È{ø^v¿â_N_¤¿à©áæ9…]¿ÞZ؍u¿í2wKø¿ïÿ⾦™\UNASNone3FGL J1747.3+0324?×RŸ1ޔ‡?Á
Šj"#Â?Ôýr—è^×?£¦Üxñq?Ó¯î69¡?ÂY/Ój,?Üñ?sÑ­?È+yÊè'm?ÕClüDí?Ça.nÏËÇ?˖§ԛ÷?ÀˆÃøÕB_?àt"-R>?²X€[Mqþ?ÎØà9áë?°Nq¼L]?ÏUÕ¼?§Õÿ>Õ¤¹?Õ1˜V¿–3?ªž²ò»'í?Ø·Xþ?§vH<â?à0Ð2^§?³´‹Øg¼ã4FGL J1747.7-2141?ûä¬+@
½¿cíÀ:ÅÛAÖÀ:õ‹QØ9è@ð_ŸLáÛ@èIåý{?Ô$yÜåɞ?ÀmŸ*R9?ðfÝR@ª¯³…S¿Ð€¡öµT¿èù›ÍP€K¿æöJßø"¼¿ì7ûþé¿Ê$xs'.¿ïõŸŸ1öUNASNone?áÒR9¬›Û?È
-þj?Ž‰PVdu?öh
‹i?Ûgú$%?Çû"µJ—Q?Õ!·ÙÑ?Èïõýa¹Æ?œÈ5|÷U?­ 'ºªŸ?äˆâǖØq?È<ën´ìÒ?Ú
¤Ïû'?±ïe9h#™?²N²;åð?šÜ
±?à¯WWÚö¯?±±š[~?Ó>ú_»®?´¸nŸHªs?r¦
ÑlD9?pr.²=6)?æ;6ºÐI¡?´á¶×fú4FGL J1747.8-0316¿ê±ü,is@)f+®´À:ÕõbLMÀ<
Ê7Ǫ@!êK¸»?ýÓ
ÔoX?ÓÞõCc'?Ó¬¹1–?ùC,Tò œ?õ`¹ÿÉ¿ïùæuë>¨?íK@š$?è6x—ÁRE?à'՟Ú%¿ç½ûm#D¿ä÷ëÿ—û4UNASNone?éKZÍzT?ÀÅ`RÂ{u?†"âœ*Z?œ¢§Y7¾?ÉiY¿q?ÀOèþú±Y?ì$ÛgÏ
?ÁÕâvr?™@Ž¯µÉ?­þû˜÷?¸‰ÐÔFÞ?½Uh Öí?çEÐ[ÿՑ?­÷Sz"?©dꕡ~T?" ר"g?̏ƒê˜J%?ªi€5‹˜%?åÌHd6Tç?¿¬¨ÇR?¦Mȝp¨?¥|…h=ü?ѝξ¨?ÀpÐ÷p7j4FGL J1747.8-3006?ÜÈP©ï/׿ð}'@.Ä9À9ÚZgT£À;‡º.d—@ Îî™Ñ!ñ@$½Ÿ2_Ï?×}Îâћê?ïRú®‡gh@ž–›¸WË@¤öí1Ç"¿ïã%Ô¥ß"?ïgòPµû¿Ø–8ù€Š¿"Ÿ\èä0¿ë¹ýßÒ¿î女©UNASNone?•ô
aN{?–º‹*9£?Æ^ÙÁk//?ÃYŠk`L?鸩<˜ÉÁ?ï6H͘?¤Ž=7K?°¹LgËÄ?ßÃTô­@ø?ÒÉíî=hè?ݼyC«Õ¦?Ò'Ã‡?ʦY¥Nž?©°‡ðÆ~…?Íò¡Tc"'?°±Y¦çØ¢?áü®}Çx?±×5þ㇠?² )
&ª¸?¦Ñä@%_?ä"ó"®Ø?ÅږÅïé?ÒN–U¡?ÂÓÉð*ŠH4FGL J1747.8-1827¿ïƒì"ß4@æ¢nTqqÀ:Qè·§À;Ê×)G!'@Ÿ6çrÀ@8âºtÛt?×¹vCS;ç?ï.À½të@ß«ºbg@é—M¹ò*¿ïÿ*b{ö?ïûd;¿êPëHD½¿äeÛ&+ã´¿ïÿÿÊPË?ïþá˜á¹UNASNone?Ä0H…;Ô?ÁcP¥Ú{ï?ÜbhÚ°	Ý?Ìò—6Ã?مrâ²69?Ë¿À,-;£?Å ÓS
?Çàìíè9é?árÊ'½5?ÏÔ êæ~b?Ҋ^‹2÷?ÊbISkÛe?р@ü½#?©%1ö»ž&?Öeè?èf?±/Nsè?ØÖÃZÈý?®ÓéŠ0XÕ?ÆõúpFEˆ?°øÜÚÍÎ?Ûýù¯ý10?Â8‡­î?؇	߬?¾˜#´¤ö#4FGL J1747.9-3224?äø]å–û¸ÀÔèÅP׉À:¾¶‰"iÀ;?"øS@+ƒ«›¤·@Ãf½Ì?ÑØýݐêI?Ûnàˆksì@	ÉrŠar@€Ì T‰D?ïðvŠ ØR¿çu5×RaÍ?˜ y
'¿ã5"÷{Í¿êDFwÜ¿ïÿüÚ±'ÞUNASNone?¼wÚSÇ7?±}
Óé¸?³ñ$æÕ5Â?®††§bo;?éòà a?¸‹¢‰}®}?Ãú·ñ…á´?¹•åj¸Ü?™¢hÜ-É?ž/ò
ã^?ê4>¼½-?ºFÈy™?ÉÔµUäƒ?¦›†ø1?Äù¿ÈÄ?¢fx'É}?ä'Ô:"ÎX?ªÏš"h¢Ó?ÁeIutÅ?¢n	f¨?­Nq´6w?—¯—´ Pô?éãÿ'b/h?§fµûbt4FGL J1748.2-1942¿Öæ½
¯Rá@ålÖÂðÀ9
‹ýáÀ;>–•[$@b'AcL«@-¢ÝåùÄ?ş£†ØL?¿=f<õÔ®?üT\É.²›?úÉ·0Ù;Æ?퍝aûÁ¿àfêþ<¿äSÇÝúœ"¿êHÒ!Š_¿Úý[?Á¶ï¿åës¶±•UNASNone?·›EDýÔ?ªLNpQ§?}þ¥é¦Ù?yA&®ƒè?ìÒwZr1?«kyGyœ?Ê30×k"?½"/^Üӓ?±"áEy@^?²('šAï?ç/—ý,?À'Ë;Ò!?Ó»()(Ã?¯sõmÐ?°·Bál¿?p ¹'…?ä!‰>?¯Â!õ'E?ÆCŽT˓?¡œ"æ˜ê¦?«7}ýÈU?–°ƒÏr*=?è»ÄüŽM?¤¤ Çƒ3Ò4FGL J1748.3-2906?ïŒïícEJ¿ãW;P8&¸À8+Apã—êÀ9Äöæ{Ê|@­õ«"A;@ý%àdYF?¿Ÿ©¾×ý?ԉƒâM<Ÿ@E¿9fS?üóâہñ\?ŃÁ–ò,?â<AßÉSÆ¿áÿÊñ*z'¿åž¯ƒêY¿ë˜ÂÚÄ¿ïÿÙi"A'UNASNone?Š¦²÷ùŠ>?ªT	Ë
Å?áJ­7?ÊÝøÁl²?ܖ•
??Ê­€ÂUF|?06h£±
?"NþNu?Û·žu†5?Êâ)Kv0?á§p"¢®!?ʚ®í;C{?¡ozßW8?Žœ>U)*?à#"ՁtY?¸Ku6Ï®?݊èùLf?·oâN]4ó?`¸@ôÛî?R5Q3Í?ÄÒßÒpÞ:?°Šãl¬;?꺏Êníj?°®ô'YùC4FGL J1748.4+1601¿ïÍÒèMd@4û3ÚøßzÀ:ÐðŽrôêÀ<K¡qÕ/r@Ɛ'ˆ(-@?']<9?ÒJ2žb×?Ù¦%ä@0ó@Àa"V!@Gœ¡¶Ê?émjf¦'G?ïý%?T©¦¿ç	¦ý…Qc¿äX,²²%¿ïþ\ý1§¿"É*gøUUNASNone?êål¤=P?·ˆÇË*¸?´Ô—±Tä?±Þ®U]º?´*¡1…?¬1®Žä¯R?èbûdiDÂ?ÃBªÊÿÛç?¾bFë—{?¿ÓRÕb!G?¾†•ÊBw?²ùtdÿÎð?ç"^iî?­ÜÐeZ´?¸upüž?œq8+a?Ç<þ	?¾?§^õ˜¦?æ9ùK̀"?¬±ºù'5?Àu…i:O?¨3.@0+º?Æ£KdÃ`?¤÷»CkiÎ4FGL J1749.0-2119?颢éñÃ@
0d‰Ø[À9…
a'ÏÀ:­y×\rÈ@»˜•±ƒ@<ó~}×?ÓÂìCŠ™L?ß¡2À¹o@ÛÐüv<?übJG¡Õ'¿à+"H×à¿âØÂ!y¿ëðÞ¤æ¿ëF®::Žq¿àÿñ½GÌ¿ïãtÿ†]}UNASNone?ÉÓK£a¢ž?¾4í à?»ˆëM¤ýç?»¸ÛgÝSµ?æ­r÷œ?ÅeJt?ÀATe1D?¼M{Q'Yd?Γq‰N-?ʁ¼L™?äJÞȟ #?ɔZ~
?ÊÒ✶'?¦ÈF•&~?ÇÏ*&žD?±w;'fuÔ?ãW|÷O*Ë?³"•à£ç?¡>v§ãbU?ŠÅQGsUÛ?»Ò¦J-½ð?ªÐÎM‡ãÂ?ëqÃÌ<?«»•
ÿSÕ4FGL J1749.6-3143c?ïã\]pjïÀn²Ð¢DcÀ:ÔK3ÛÀ<j¦gv@`ÆyvŽ}@åF
¦L0?Ðô»¾²'Ê?ïr7Pþ@ù?R%g@=‰"~¿Öy>‡$L?ï5ÞUö¿¹_ò.+¿ÜB‡d
¿ïßëìd?ê:#aÔÜUNASNone2FGL J1749.7-3134c ?±¹'kj͵?°*;ëŽ`?Þ•6ʾ|?ȦWÆÚé?ÜÏnZŽ?È'~î@?©uÓ¼E?±º$8Ý?âQ¥©¿?ÏæV•â?ؚ¢Q[Ø?Î8pN›?Ç»®¥Î‰?ªô'ãWë?á`ð¾?Œ?³vÄw=&?Ñ`G0š¨#?¬‹x?½JǼ?¬"!Tðž?èAN_Šu?¹{7îÀªø?Àq 'IÐ?®ÈÆñ£Ä4FGL J1749.8-0303¿à"ˆˆODa@(q[Ývh<À9.¨mqóbÀ;\ý#¬­s@·"CñòK@FC´g?¸¥.ßL½Y?Ñv°@O%'@}"Ó8÷˜@2A~$ž?ﹺAn_¿á"¹"K‰¿æŠ"XŸÔ¿çu –
¿ïþ@½Šd¿ïç0ž-}UNASNone3FGL J1749.7-0305?è""[¦ì?À«Ø‡ãAO?ÂbOkM \?¹¦|H%?º&ÆL3ÿñ?²÷:9Ô?Éډ¸Di?Ã.aˆÂ?ã^ç!‡§4?ʽ[çÂ?È©Úq)Æ?ÁFʸh?Þ="3}Å?³q•«b›"?Ñ5jaqûÍ?°ž™"T;?ЍkŠ†o?¬fJôV×?ÄÝHÜÒօ?œëL¿lJ?Ø5Í›3‡?¯¯»"ö5?Ý[ŽŒûa5?«ø~º%†y4FGL J1750.0-3849?ï¿ÿª£4ÖÀz)³únÀ:FdÆSÀ<ø´²#Ô@ÝâF܈W@Xô›Gïƒ?ËJ}|­z¢?êÁLÁN¿V@ÍäKjb@šº†N8G?ìP¾´[<¿ÛÝÉtR¸4¿àÃ?O¡(¿ëúç\›Š¿ïþ'Ý¿áŠ¯ñʳUNASNone?¦~Î:hð?¦qye;Bû?á¶9MìIo?ȅ‹ñò\Ñ?ÙóœÚlÄ?ȈÄÞ"?¦Œ1œ}s?« UƒüÄÒ?ã¸=Æ@f/?˯v~´®?Õ¾mK£ò?ÉÕڐáïé?Â
´:™†?¤PûÉ=0?ãhlmõŒ#?°,(\cç"?ÏßC"ï5ï?ªá˜ù?«Q</–×?[mÜrY3?ç¼L÷±£m?°˜U´
 ^?Ê:}UŒ˜?­U™g2e4FGL J1750.0-3347¿Î׀7¦hÀ
™ÔttFÀ9Åét£@À;HöHÇ/@\ÜÇÁ @}N?(3ü?Ëøg…JW<?ÑUA8Úg@†&oÖQ±@¿"²²oS?ïüë¾TŽù¿è–µ¹ŠÑ¿É!"ßù$o¿åÞjNRsj¿é±y?%3¿ä¢W
--UNASNone	?°ñϏ5d?§
ɍ¹ÄÑ?@NÆLC7?†Áô¼¶?ílÄÓèG?¨ÂóóL•?Îr‡á¦Ó5?À_È®À7:?'m$")Öú?˜HëãÀ?ç×ôãtü{?ÀrR+ö?Ò~'…œ…?¯Ž§pç?¸ÃdhpX?—FímÛ?ã¨J0k¡'?­°ê"¬\?Ϙ<^Ù8+?¦waSHR?¥#ŽÅß?‹Oÿšùƒ?æÇÀŸi¥˜?§Œ¥n¥º4FGL J1750.4-1721¿ÞGž`cÿ@	$kðÀ:òÕuûÀ;¶၏¸@¤X[¶µ@ 6^`Þg?ÉϚ‡€<{?×ý¾¼éªÔ@»A®@ñ@…šPΤ"?îðÉ@Ñ+¿ãÁ9»ãp}¿â=d_%)…¿è_‹*ì¿ïÿÿ" 5•?ïÿû-2h2UNASNone?È6¶Í¿ÂV?·*¢éƒ©?ÉCÃh€àì?½ÁOc{—§?ã¡aro×0?Â
•?Iuz?ÍjԟÎÒÛ?Ää‰>+y"?ÅÁª0˜Ÿ?ÂÛnBìÛ?ã4àKæ#ƒ?ÇNg'zp]?Ñð{cši)?©±y捰?Ì~Àô/á?¨[1{ù?ßÐ$"Ne?¯j³8d"D?Ê9àHƒd?§Éû}FÊR?Æò­€^‹Å?­'‡FÃX?ã´ÜÇ"?±MUÇé°h4FGL J1750.6-1906¿íkcϙl@Q€Ø´À9lm½r¼¶À;	:×lc@"!"9Å@þ7"«üs?É·¸=žœ
?ÌϞxÑx@}£!ØG?÷ô›ï	?ì4јäh¿ä×ø¿Äс¿é8Ï>ìúÀ¿ã»?Ï¿ì^ý¼Xá¿ïý‡ŸñøUUNASNone?ÄÊؘ`ʲ?¶;T±z¦?Ê%HÄÌ£?¿'…Þ£Z(?äI@‡¶š+?Âr¹Êgc?´eØýÈö?²ïéAL`¼?ÒǔEº;?È%BÃw½?äz½I`?Æ¥oCãì!?ÍÑ,äÞÙì?©Å`÷T³_?ÂÅ¿'¿?£ÀwA9pÕ?ãÚDægÃ?®¯z?šº "'?~ä
©ªª`?ÊÒ@ó×É?¬Ïèj1Î?èz}Þ¾mþ?¬Ñ'/¡4FGL J1750.8-4405¿ÓCè*SïÀ!Jæ…Ûv´À:gþÓ°ÝÀ;àZ›W	@öä¡TÎä@Ò	Å{Ÿ´?Ðúk _pÿ?Ú?B5.µö@ž$»¡+^?ú¸`ygu¿Ø-³Âd¾ñ?ïÏ¡ýÁ6¿ÑµA*l»¿ä;ñb®K¿ïÿà?Æ>"?ïúñm–UNASNone?Í!wÀRû'?¿GǹËô?¼ïñfñ?µ/E(­ó?å£íbù?¡®&,Dî?×!¿—ÈÇZ?˘.õñ©Ò?µÅzfµål?·¡&D
?á¶pçDߦ?Í=::N]?Ù¤' ÞH^?­§EF½[q?ȤW·ÌS]?¦­ŒmU%?Ú	R;ò?­,}Ðy&ç?ܯƒ-͑?±}÷3Û1?ÂH揭¼?¨¤ˆFî?Ú,	‹fې?³>3Lv4FGL J1750.8-1246¿Ù2"%°‹@å$9›,AÀ:€T–ZIøÀ;©Äÿxñƒ@2ް@º<÷T?ÖVԍ‹n^?ã<¥7\ @"ª^ã»&?÷y¿¹†?ïÿÁ¡u†¿à}i[
¿Ø|1©Æ7‡¿å@p"|ח¿ïì[rí]f¿ïäu_þmYUNASNone?»ñô¬h?T?¶ï5·Éï?£p8"‰ö—?£Å|Çߋý?ëJ½â*X¬?»Þl®{*?Â݆àúõá?ÂNì:~ž?ÏÝ»i3ò|?ÉÞÙ´cj?ãQ/mtEé?Ægÿí#?Óû&iã¶~?¬A»EÚêõ?Í&,`dõ?©¸x•²<?ÝqØì?®1µ¶y>
?²-pãC9?'ú a϶?ˉ·ÛÛb?±?
1Àõ}?æØõ ¢?²a.'o4FGL J1750.9-3301?ß|0®"ÉdÀ¡f>ù:À9º:NÀ;9=e¼{@Æ<幃@–õw/?Éú»¡ w?ƹ«R5Ø?þ%½ÿªo«@v:2€Û³¿ë<":µ´?ïñ@x@.¿æo;At"|¿äf†a®pÁ¿è›
²ái¿ä5M>ÍPUNASNone?ÆR²1r%?µ*døér?¢c][™[?¥"
}Ïý?éEñá¢?¸˜éS'l?Ó/ç
Z°¼?úî¥?…h#âL?"Ui'¥†ù?åãá83—?ÃZq5‡?Ò¬ÅxX?®)‡ kû?³ñc'ãa?–aæèù!W?äuÄÉLçg?­Å¤27;?ÚpXù?©[^¯ðæ7?¬K 	ãŠ?"yÊ  Ø ?á5@G5ɬ?ªNå'óâ4FGL J1750.9-2655¿åý|ô?"¤ßʚ1À9)LøW>À:ªo ¡Ë—@Ýèuõ¥‰?ÿe©Oð?Ϧ-ü'6?áÅ»ámÛ@ÛxFbºà?üAmwþ?ïþµ}$îÍ?è­½¨l›4¿Öàæ?³¢¿ìzD5ë¿è¥Ùä"s¿î|¯þàÆ)UNASNone
?€ýы±CL?{@ڑk>Í?w@<·8?}v]†d?@c
Ã?†«èZ×Éò?²îDCD?·"zô.°¹?¼'½®ô?Áëeᙾc?ê8ì*™?ÅïwÐ{A?Û"˜Â?¢ÒQ–¹\?ÅF|ó¦\K?¦5Ê ²/›?åǘåá¦?ª—Š{Ýðâ?¨5"+*i?¡?·å<?³ÙãÏÇÖ¤?±è]aäëå?ìqÄR…?¹@EïÏÖ{4FGL J1751.1-3455¿ì­ó·X'‰ÀUiR‹¾À9ø'õ:ª À;i²KAFò@_fPÁäf@ÿ#a.?Ê´®ÈÕÇG?¶)vpõ‹ˆ?ñÛCˆ×?÷WdZÈx?ïŒ$Ñp |¿ÞâšÎÍÙ¿ì{´ÚgÀ¿ÔBe"oä¿ê±ó˜°Ý¿ðUNASNone?ÃÄ@ú¤¿?¹âš–™Æ€?w'Í"¶ö¶?ˆ—D¦«?êßê]Wèã?ºBdÌ:"?ήª-$rI?ÀX´ÞÇ?Ç?ŽÍP¤£¹?–°PAÓ|E?çÙ 2$U+?Àt$20=?×£"e7ž§?¯[ÂÓ%7"?±sPý"ä?"Höòxø?â­³"+?¯êOÔñ#?Ñ+ÔG…¢P?°­ •=Ò?¯[36	?˜½ª¥ýü?åtdYËx?³C~ÁZ	'4FGL J1751.1+0109¿ÑÏ}T?"@+ÙØ@žUÁÀ:E,YûÀ;°"L*zþ@ë"Ò/bC@œ'W…øÓ?Ԁr¡]2`?è*±^Ý0@Yàâi?ùøYMN<y¿åÚâ9E›ì¿Ý¿‹0JJ§¿èK"¾h…û¿ìœ.¿†S¿ÞÞõöÕ_¿ïó"כ\èUNASNone?ÓÙºaéX?Ä¡»è"¥?ĵy7mé?¿K¥^:·?áE4ÔóÉÚ?ÇFî‰ìâ?Ù*{¨=Äð?лŠ©}P°?Ù3û]Q?ÑÍÓa9ÒÛ?Ë¢ ¸ÉÓú?ö|ݤe?܆xûŒø?®è낪o´?È8U#á|+?¨«×"Û!?×]]Z´ó?¬ªwë(¥¹?Ä{èÓ"öÈ?¨0Œc§8?Ñ$oȁ?ºÖv1·³ý?â^s"S@
?¹KÞ¦ó%94FGL J1752.0+3606?àóm@:î®ÀrKwÀ;nƒÚ³ìÀ<ÎI2xù@ ICF¦­~?þâ¿b€þ˜?ÐÂHyìU(?Â+ÍxÄ6ü?ó¨(Ãm¨z@»Ã>-¸?ېR.9#? El¿ÐZakTã¿È(aP¿íXØãÀ¯?À[˜·§wUNASNone?îÕCÈÕ{ž?£OæÈU;Ý?wH¼Ð¹ã?ƒ
vMDË?Ÿ…W±,È?¡±yœ'a?ïzTó‰þ©?~9ÂMÂ?T/b՜?c徝"?ŽÒow"û!?ŒyÁ"jG?í	¼š&›n?›|—šÜï¹?'"Úc5ö?…A	è¿?³öø2W?–¤q¼Lޝ?îô"ŽO è?…æîvX&"?ùﭙû?r!MF—ý	?˜äq>Eþ?'‹¬6唦4FGL J1752.3-2914?ìR×ãk¿öž²r®sEÀ93âÏòÀ:N:†
˛@ÊØ"ì>,@zªÁ	J,?Ïfކ]§¦?×Jë I÷p@	wß 'á?þZ2H|›‡?ê,n¾#¼ž?ѺÔýÐ
¿åøÙÀ¦"ê¿ê7ÀÌ
Š,¿é¾u†"Ú¿ÆÌÉ\Tê"UNASNone?¡-¤®«"‹? Ež4§%?°ËUuZœ?±Ý‹Ø°Ñ?ìÓ»qbƒ?¶)d£q7u?²ò¤§\"?°½ܳËË?²0àÃâø?±ÚñRèÔX?ë[|2˜?µÒ•·	jZ?¸ØÍ>p¤ó?"õLá?ÀXQ*êÝ? +¼Ææ¡n?èÎáCç0ª?¥Ù<ª'?ešÐ"Fÿ?xh
ŠOH?¹À!ù™ûª? ¶&ç@®Ñ?ìJeUŒ7o?¡C§éÂ>4FGL J1752.3-3139?îË^"'À ]ˆ¿À9¡w·ÒjÀ;HóŽØu@DPó7š¡@õö&bjX?Îê—Ä'P?ÐY0ó½Ò^@uH#…@F?ðèҁӿìTS^¡Ëí?ïÜùjºˆý¿è–"ì"¿æ•BA˜ü'¿é7zàÆÔ»¿ÞR†à"d©UNASNone?ÆLœÕZ–°?¸‹D'J—­?³yçì*Ï=?­ÉGKåKƒ?çý›Í$m?¾ÈΎüу?¸k]ªë+‹?µ"%b*^?¼†Å»ÞÖ?»YsbóKB?éa»"&¿Í?À@Û{¸W§?ÃΡÚò-µ? ÃÊ¿·Ä?À>Çì)A˜? {ˆ}(î«?æü¥Ž9$-?§Š5Â'?³7¥l
?•>™§R 4?ȕõÃl?°9¡/Â0¡?çs š‹w}?°Ö@ù«Z4FGL J1752.7-3040?Ùg#~ùôèÀÅ«ÀãŠ~À9¶4EêPÀ;?ª9ú͑@؂Žs@–üõ‰"?Íi#šŽâ?âAº°j–@¥ò`L–?÷IŸsxGº?ï!FÁÛW)¿×Ï?"ª¤Ú¿ÞïåÿÏ®¿é¦2Ï`%¿ê€™'ódç¿ïö×B®\UNASNone?"Ü­_Rêø?yg<1AMY?¬¾Ï9t¹—?¨ßÃldr?íà Vëhº?©?¹ÇEŒv?®µåìÜO?¬·×€m?Áòh¥Z?Àœ™ãûÁ?é˜wÑýã?ÀpÂN°8?ºÃ(­ÙÑá?–Vå›o?Ë6¶žE?¬@MFÅh9?åÙíB½ô?­Ê7¥KûM?–ØáÑËP§?xY.‹|Ð?Ór²æúcw?®xÞǍù,?åß}ôs¿?¯M-ÎÜ°‹4FGL J1752.8-4449?ûÞàBóÀ"¡ÿ´€¥­À:9·	ìèÌÀ;éBí»YÞ@—M;@3ÁÎl	?Ç·&'?Ù_™ãÁZÿ@çń/_@KÐÈ:?íÚò)}§Ì?ì,â·Ý!¿Ù( ú"¿ã	Áv,'¿ëÜ>"Ë¿ïû¬áxUNASNone?¤T¸–áwå?—ß8ÃÂ?ÚFïé"ò	?ń6›ŠÅ?á—<Ïo}?Å]×ÏèK—?Èø®ò•§Ë?ƒ;
ê0?ÒYûR˜?ÈßEÆ-ö?à"Ö»SlÂ?˵Èœ÷?Ы)|}B–?©»öCG «?Ôß½}ówÙ?±÷'ÍBöN?ÚuE'?°Olä÷b?ÍÜÚ«W|?¦&×r¸ÀÙ?רÆқ
û?²Ç'1`?ÙhË×¹6Å?¯£¯tËd4FGL J1753.8-2538¿é÷'HD‡?À?^¥&ë|À7´ªÄdHÀ:L$BÕg¦@þ¿e @ìÊì"?®c_/n
?Ô/ÆÂÃÖ@#š {5?øƤfý5?áÔS»d?Ù0W¶ :ž¿Ò•ŸäâBU¿â€Õ}uv¥¿ék¡~•\H¿ì¡¶hÝ9,UNASNone?iD'"…?[ú¼'Y
£?â.ÅÍÕ;u?ɬG¯Ø4?ÛpkÛP€?ɞ7!"—|?p§½–ÜÆ?y:¹®vc	?è{€²9.ã?ÃÁÅD˜9Ä?͌đ.‹?ùØ;Ñ{¦? Híôbt|?&1D©é?ãAÿ!<1?µ(Ìn}?×rãÿG9?´™~o,úÿ?Ed0Š?2ÇÅO¿á?à@tã2ûÎ?»c«âô?ßt"‡'ð!?»fß;siF4FGL J1753.9+2443?î'Gœ\þš@7û¨'j©À:2@h¥ÛÇÀ<[š'Í¥:@҉¹ý'=@ÅΞ^$y?Á"K©¡¤€?¶@+"-t?õbØ<l˜@
ÒÐ]t$?í˜ø‰éù-¿ç$‰¿ß~Q€ž¡¿â7 €=¨¿áXK»À5¿ïÿ¬ÞoâfUNASNone?ïðzÕÉ¡?ZC®v¢åŒ?3¦`–‹À?9ƒ{½ÅI?Z ¼GG?U¸þ±H,?ïÀ/ô€.-?~ÆÃûÂ!?;µª M?O¯ûo¼,À?~,«褸?|Ñ/‡x¨?ïw®Lp?'ƒŒ*¡iÞ?n¹H«}Ef?g-m&}?™9á!©N?€D'€©•T?g>XÍ?nšåoÜ<?YށêJ%?C™€H¸ß?ˆ#Uó&c}?lDZû鸵4FGL J1754.1-4333¿ì'Ö_À!ϪŠ'¥aÀ:åªô4ð£À<Taä ¦i@!®ˆ Ø?áÔ"°Õ?Ú衾V?èçԐ­?þHż7SS@ª¥¼'—ó?ïù
ãˆÐô¿è¤±ÅàI¿î½_œr½?Ë®¿Æ~ÿå?Á4Æ[C¿í¥qß@lØUNASNone?×%"Ñ3ˆ!?É\±ê«Fª?€gIq	L?UWiee?ä+Ҋ@wË?ɈPîK?à[>½W¢?ήR@÷ÉM?p¾Ë³Bäª?Åa¢P?߇V"Å+?ÎDºÊ3¼–?çၝ?¬š"I§_?œ¯wºå?‰_U: €J?ÌåÊ®œê?ª;óP‡ó?é¥=>Òâ?¼FJ'y7U?D;V•'ž?SQÌ:=t?ÉWoú®ã?¼K±®À9L4FGL J1754.3-4443¿¬ÔìQ³À"ûR†µ'GÀ:x.åƙÀ;Ý Y§;@NµÖ\@Ðä¤Yæü?È;>"õó?×Wôž"}@‹š°@2+5㼨?ïý˜F³B¸¿àžÜd…¿áø#'¬?¿ç²ñYt¿ï='á>sÙ¿ÕyF<û3UNASNone2FGL J1753.8-4446?£ÅqQ†eË?¤;ünØ?ÂýÜmzí¹?»0…CFt?ê1ψÞ5?¾]¹XštP?ÎOe¯*¢?ÇäÓ/Óoã?ȏžì	Iþ?Ç& {v	?âH>Ù7âØ?̵mU2ë?Ël'bZ-=?¦O/ÊV?ɚý Àî?§'™7)Ù?â¾6¶ÁDu?­J/ÑLA¹?Á›3Yá­?–ùˆúÛØ?Ð6Ä%?¨ÌÆÛ<¡?ã¸~*GtÆ?¨™GY¦4FGL J1754.3-2915?è~­|ûSH¿üÙ`sÞ.À:<Ñ®³ÝÀ;Ï!CF¦­@V'ýž%ð@•§Yu½?ֆm'dsÈ?ïâp"&ñ[@c§@KIª?ýž€ÌC:?í«j¿îþ@5û?çÕk׿o¿ê¥_Ù.…¿íÛÇ4ÝW¿éñ\~†ÝUNASNone?¢Ð&ÇÇ:2?£$wsΛ?ÏÏÆi?Åèý#n?缟¿ÚÃ?ƬÌiCXÙ?«q9"½°?±±meòì?ˈυ¢N?ËDŽ@´×'?çkõ
þÑ?Ê|Øí2#î?ËÀjðnua?¥Í@R¯¡?ÒûÙæfâ=?°7wdxƒ?ß#ð¡aã?°‹í¸u?Š7ã},I?€'á•ÌÅ_?烯nPë¼?¹^õ¯J?Ð&âtÆ@?Â@×Õé¦4FGL J1754.3-3236?îMK°¶hÀðƒB?@À:ðéÇ´À;}ƒvA¥½@þŽøœ@·†ªØ?Óý31…´
?çÜÄA
Š@~}ÖÅt@7§î&!?í Ɋ"-?ìT4ÀQn¿ä3¬Õ¶€Z¿îF—> Y¿íõ~†mÿïÉ$i¢UNASNone?°¬›HKû°?¬ƒøþšV?Ã÷g–¢h¶?¿9à5ì?è쒱Mæ\?ÁلôâÑ®?±žñ€tž?´+âø֘…?Öµ<8£;?ÎRG7Oh?âqƒÂÕ+î?̓ØöR)z?ÀCÓ/¨U?EKokQ–?ÑÐ÷L\£-?°ÔZ"V£t?㏎DT?±+"O¿µ?£VpÃC4²?‰›21óÒ?ã[R8ð)?ºÐ Â‰,?ÖލÛ%¹?¹5Ì &Ȅ4FGL J1754.6-2933?ìZ\áh¡eÀœ˜†À9<;¨LºÄÀ:ѕç]qË@ƒÅ[¿Cw@á';×F£?ÇFŠ¡Y,?Ý°å:¬Ï@¬$=Ìê)@Õú¿ïàk]¾L?ïÚ¶š[`y¿à4v)R	¿æÉúŠu9h¿ìÏÝ=]X¡¿ïÿC*!<UNASNone2FGL J1754.1-2930?²ç~‰" #?§¬zhu;è?Ó/em^?ÄbëÐÿù?ä]xo;?ÅœÁ@?¸í;¸S?·Àt¾?Íföb/'þ?Æ|Õ‹¤W?创Ýß?ǟ{E?ºÚÈÆï;ü?žÆÒNé"N?Ö0HŠ{?´j¨—æ!?ጂ¢Úö?³_â˜6Ä?¶ÛÄÜüç?š€¢zU@?ɗ½˜"?¯ˆýQ`?æ¾ a]{^?²qÉ×[‡P4FGL J1754.8-3200?ï¼î…À
*s±éÀ:€aº/;À<AÎm¶¼À@zS¶xM@XÜ}Cø}?Ò	}!"Î~?ïö@líüÈ=@4¿ÆÔæ!?í+ž{ÝÇ¿Ô5edd¯?Úø¦¥×¿ß½Á+®Ús¿ïýÝ¡s²?î¢ÊšÃeEUNASNone?ÅÁѓo[ ?¿ÚùmÔ,\?ÎYk"?ì?öZñ‡g?âù(@C?Ʀ­Ê«?¼^Œxñ1?Àh.·Ô¦\?Ðä1¹I"?Ëý°»Ð[Ó?äy¢"=?Ìúw™ŒË
?ћ8¾ó"?²l…´È?Û¡Áû.ÓÍ?¶ÉiŠCxÄ?ÒÃFÅ9?¬üýÝý3?Ê|§Æ´V?´˜ÿhå@v?á§ì½'òE?Á֏S'ߏ?ÎäFa킘?·æ
SurÎ4FGL J1755.3-3937?ïð#®ÛËÀ žý†¨üÀ:Y‰SÑ8lÀ;5^†ž@'êF/dG@bû…Fü>?ÚâLÒ?Þ]C½oÑ@
S½Ö.u@ÚÊö†?ÖªtÞ#aY¿Ð4à²\Þþ¿æ<˘fÙ¿æÎG P¿í9Ž—¿ïû
¢ò)UNASNone?ÄÞ+ô/Ïu?¸…Ô‡C¼?Ìã|v¨'?À÷4ÚZOÏ?ãÂ<#Öb?Å21Ì C?Ó½;1I´I?É4&k¸Ù~?»ºüÝ?¼¡Þi˜?⽂cƒÆ??ÊðÀ­8Ø
?ÐÃ(r""?ªR Þ<m¡?Ŷ+üGR/?£>®ÅoÊ ?â0àÇÜáî?­4ØoÌÂ&?ÑÐ%Ÿ­F?©"Ú"Ò?ÀõBº~-â?­ºøƒ(F'?ã>Ç>å?³€ž'4FGL J1755.5-3734¿Èi8}ÊÜÀÂu%F
¦À:3qxéêÀ;´Ç%Ãß@àÃEJ7@¹}£~?Æda¾áҘ?´¥sl‰@0?ðËoÕzñ8@å½ïD¿í
Û¢R¦?ïâN>Qtg¿ëô…þ²"'¿ÙÕp_c'Ì¿àÍ]ìDaY¿å3TÁ"tŸUNASNone?Õ݊Ýn	?Âö¼y'³?ŽTþ‡…xÎ?‰;K*¸¯õ?ä—æ—*å?Ã\'/ë8I?âúuNJ?ÆL³"|Öâ?d'f#ÌPÕ?rܶÑ\Ò>?ÙâÖIŸÊÍ?Æ4si1E?Þj.ýу?²ã"èý9?§Àš×(€?ŽnÚêy·'?ޝÓ§Im?²0(÷ãß?é^Šæá>n?£êse'ø?"¾ÍÃ¥]5?€CÂÆ:"?È
ú¬Z¢?£ÐD<œ4FGL J1755.6-2050¿ÑÞÝN,ç@'¹"ËÜãÀ9£B,Ë:&À:èî4%¡z@-=¹Ic@$ ]Øù+?Ã0ÞÖÏ/¿ŠSa?Ͻ‡?Ç×[†Žz?ý£øJÛ?îœÂþí±I¿á±—¢H"Ä¿ë7Rè`¸¿æd¿1ٖà¿ïÿþó…õ?ïÿùŸé"ÚUNASNone?Ú=Þê×?ÆOu0Ÿ?˜h
فî?¢!<Z¼­m?âЩU¾…?Æ Ûóº?Ö×,QÛ'?ÌPÔX''í?žŸ¢÷ڌ?ªQ†Èó	{?ãŸlÆҁj?̱­á̶?ÑØT8Ù?­Ã#z!vÖ?µPj¹½?—ºŒÿž?äiȝ,\¯?®v¬?;|?Éì<]yEÑ?±S·!ò9?˜óoøTí¦?ˆ…jSr^?è½Uhß?±×A±Ô¼4FGL J1755.9-4009?셕²ž<À^[ÕêÀ:'ci[ä,À;±£_9M@/ðÚs(—?üè˜`´v?ÛúgVPo?ä%+¾IÒ1@!='AŽ@@¡~O'7Ë¿ïÿñh?ïþ¦>½·¿ÝÇv¡œó@¿â¥ýàÀõ~¿îßô╋î¿ïÃÆ^‰UNASNone?ÒÜ5Î9Æ?ÄéºþÒg‡?¥˜¶MÅ^á?£¶£õÃ-°?å8Y´ê/?ÅÈ5äM»?Û­3ìRb9?Ëpʝt?¡*ð\ºýu?¨Ðóøç1Ê?á·?Ë^Ņêš?Ú DÒ+¶?¯ÿ)úhîL?ƬfYÏNã?§DÜmY|?ڐ¬ŽF,Ø?®oڗ'?à'xzØËü?¹ž¢/?¡ùUóÕs?˜×‡î-Ê?ܛäKÓÄ?»OòØ'
ö4FGL J1755.9+0953¿Þsñ¶®[@0Åè´k­À;\Þê¸À<·k;¸=@"6°î[¾?úA
a'Ï@ƒû¶Å$?ïEj7¬>¸@¡¥×•~?û´Ê­7Ü¿îÖ¾ˆfko¿ïÿë<ú\R?ïû!ô›?ïšT	lL¿Ýº7~œh+¿ïþ"?½…1UNASNone?ìô1È?½O,{1=Ú?‡Ã"
ÃÚy?¡Sÿ9÷‡#?µfg,´?»Ê÷'l6?è1ÝÉ«Fž?ÓîçhÍ?Ã5ØÉÒ' ?Ò&VÍä?¸`{Õ?À'*‰"?ê÷QÜ1ð»?§5p$¶ÿ?•§üQ‹â®?†*果Ñ?Ám¹À¼?¥ 6˜&ã?ë~U5çàX?Î1‰IŠ<?x5Ñ<å¾?¤Ê‹¼Àu?ÁDüžyV‹?͚%7Bgr4FGL J1756.3+0236¿éP²7Ó´{@*áŒâÑñÐÀ:#}At>–À;ž³ì+6å@‰Àë,ß@¥½"J¥@?Óm©PÆÂ?Õ
ßâ©-
?ðßXÀ‹v@ÒU%v\?ïïB¾¤Ø¿è=-rH¿ìRþtå…*¿äÏ/!}¿ëðžc,ö?·ºú½Jù£UNASNone?ã>-¼…Æ‹?ÇF³ts?șv9̋?Âa'ŒLΎ?Ên7—¯H?Á Òg³?é<á¯ûí?Å:'3ܾ?¬¨av㧨?´×ºo˜?ÃâÙ‡&d?Àá*&<x?ßàtÛÆÏ?¯z|¨K4<?Ä*HBВÍ?¦B"ñ?ÖÐûi»ïÊ?¬"9‹ï?å"eêQ5?°ËaJ]çm?©úƒÓ?'Ï®«²Ìz?җRðÚùÛ?°lèŸá˜Ñ4FGL J1756.6-2352?é":ÑHm¾?ÝÙÓÛߺ:À8"d鎤sÀ:/4q÷"!@ҝ{PƒP@
×^÷\?Ør³üœHK?Śx§0°ø@'Í|õôä@"\d"ä×?íQ`_¼(:¿í?½ÅGó¿Ì7¤/¿èpó‹(¿åôÑÞ¯xS¿ä@GƒLP;UNASNone?›Ki²qD? Ò³õ?«ÕƒAöŠ"?±kFµ?íhKГÎ?µå"Äo'?¤Ú ×8µ´?¦¿zßÃ:«?§7
;xL?®cÙ·*öþ?í>Ý!è½!?³{O"?µWlÒà'?˜;°¿·‡?¼Â»0—¸?¥e3£ª?éÄbúÿ'?¨áý.èvú?˜Ht"מ>?©™+zb%?–I0Ú­í`?Á6u4«?î‹rԋӣ?'"Q"¨Uß4FGL J1757.1-1926¿ïêë¥øD@Ķ¦ڝÀ9±RÝóe¾À:þ»dÅ|v@9Xo­·ß@6¡|¼ê?Ñ"0?ÙÛ¡¦ÙH@Ž¨¿§J\@Ç²0¿;?ïñ1Ñ3cÛ¿åÏ®&ïX¿çÓû_‡O¿èÃ^¿ìr±˜"à¿ïÿï¤h)µUNASNone
?Å	•CÅ6Œ?µ‡ùwI5õ?ÃÃK¾×so?»¥õa®q?åÌÇ¿XՁ?ÁN…"â·?Ç'ºöw…é?Ěw&"Qr?Ãê©Ò‹Áš?Ãk—ƒ?å;fÍ¿. ?ÉI¼"gz?Å_z÷"[œ?¢pûîù?Ǹ.­<<q?©.öÜN?亖ËÙý?®±ÒŠUuZ?¨yÞºóc?ŽÍÝáôÁ?´Èœ ÍÚ0?š8(@qÁ?ëßN7‰? h¿8šÍ4FGL J1757.1-3554¿ï#æÕó£7Àˆ.D¶é6À:aÀ¥wnÀ<|Dôü—@º÷dP±@/¦¥ñ—?Ìr‰µJúû?á§ZS<=@áè¢ì(³@:ßý¥?ïþ¾°nÈ¿å$@ò8— ¿Þ`\̉°î¿ç¸A¥f׿﵂˜Ì@¿îñ›MοìUNASNone?éë[!'þ?¶=ï7V"½?Å3EDî|Ì?¾½é«øvÍ?åȳ×ü
?ÂÈE†Q¸?Ħ¸Á?»¥4•hÅG?²>çƅLå?³‹;À΅?è±ùY)Ñô?À¨¾¬¾:Ù?ÑÙ}j¥×?±#m~ ø€?Øj%Ö%?µ0\QÜqÍ?Õ¼]•@?®ˆÍ±k•'?ҍR/`Ê?¨àý‡§\	?ÇCR"¨>?©´y?$'ª?àè'CLT‹?°ôÉ«4FGL J1757.1-2848c?Ĝ§±ñeoÀßOC427À9¸™9!ŠÀ;!-w1@
2AEÆ@ðÛâêE"?ɇø‡eºo?Ò¡ÿěÐÖ@	Gcä«æ£@«.4ä³?ïã²,¿Üáàš´÷™¿äµü¦¯,¿ç´<G®ë:¿î2BÝË!Ò¿ïÕ ÞœØéUNASNone(?¡Q¢"g¼ç?šÖÏÚ££M?«Úk2Vš?¥V¡(úDU?í-?$"7?«Ö;WG0ã?¿øq@–â?´ÚðVõr^?¦;^ŠZ‰?¥"'°sÁ?ê;ïG'Ä?·¡™-E]?Â09.ð?Ÿ=zü#¿?ÃðkŽÑRŸ?¡‰Aþ\A+?æwÖЏ"?§lrÊY6¡?¸Ë؟|Nö?—˜Ôêlñ?»ì_ž'?šL²•u?éhøø>3_?¢V8£C'4FGL J1757.4-3125?à­÷"'äÃÀ«ºÅcLÀ9xäû—»sÀ;‹w·Òj@²:öËú@›´áô|>?ÀÁ_Eà´á?ÕàèãƒÈw@ߒޔum@_5¤ ?ïš½ÐZ¡¿ŽWÚÌ-¯U¿â«)yv
£¿æª)¿l ¿îà÷Ií¿ïòè ¹UNASNone3FGL J1757.8-3126?±SÔ¯´?¤ÈçŸH
?⛥¢Éð‰?Åñ&Õ9õÈ?Ösî8vó?ğ¤?ÄN?³I™câž?°Õ¤úú?֓PáñOÃ?È ‹ƒMÂs?âM4»ÚÛË?Ȍt²ä¶?À±3¤>?¥¹Êï¨?ÜNÇø8ž?·n‡.ùÚ?ÛXž&ŸxÃ?´üú‡¡à\?½ál>û$3?—'?9Ç#Œ?àø/•Ðà?²‹%ñ(¹u?֗h'•3?±ß¡(Í4FGL J1757.6-2731¿ê¶I-¤·¿øÐÒëʾÖÀ:	 »aj~À:úÑ9C­@†"'&3@mâÀT?ÝlRƒÛlM?àëEþçÒ@
x¡UO¾?ÿm>ô‡|?ïó$Oj¡_¿¼‡!F÷‹<¿ÝA"Šfð¿ã¾¹ä¾¿ìÆÝ»²s¿ïïë€:ÕUNASNone	?Œìæ‹Öm? •ŸkX;m? ÖmÑïÍ?¡·]2¢|?î'uˆ±©?¨&÷rÝz˜?»Æ5T¸?·".àòìÝ?¡È7!%?¥OÙ+'ÎÂ?ëvß×ÅãV?¸¥Ï8ÙX¯?¾Cï÷
øÄ?™o)ñ¹?ǀ±0ˆE?¥"ûŠÁ®?æWU»×?¨Ýïێ¢­?¦æ›'«?"ª"ÔcH¤?š¯q'q?"%"FÑæ?í¼GA½õ?¡(tžŒÃë4FGL J1757.7-6032?ïý¼ãd'¥À1/ס<%JÀ:4Ú§€âéÀ<iË@ے@œÝ‰š?ú
¦ç_ö
?ÆÍÆó?Û]õ¿	j¸@³·õfI?÷Ïxw
#?ï×táSl¿âYbqå ¿Ó™û꽿͝CÝ¥b%¿ì}y¼"€¿ïÿßéà
UNASNone3FGL J1757.7-6030?Ó×Ñü‹?ÅnÿÞÅz~?ä—I˜t]?ǃёr&?®t§îdb?¦}×0€š?Æý Tlæ–?Å}*Ö>?æn¨öNôX?ɾI«"¢Ò?¾w¤®?¶þ¤¤‡?ÆIÑ@øì?©§r§Ùê?åP¸ˆ5AZ?°3ÿ\Ïj?ÄsLž2™?¥;	?[æ?ÎÿïÂù%?«ÀuÕπ?ÚN_í'à#?º, =®ƒÑ?Ö1¨1[?´È†k`-«4FGL J1758.0-2953?ë Hj|öÀ0ÄÃéÏÀ:uK8¶ÈÀ<Tlô!-@-¡"¹ï@ÞZCBtð?Ò¥î[è´	?ïçùÿ4þå@U ÃÄæ?ýYnîöt¿îë\‡Ê?ï8tP3ôú?èëÏO^¿ã ž9%¿ï1…ý¿ïþ·á-VûUNASNone?¤i™ŽØ÷¼?f ¹«©?Ý}ºÉ"/9?ȃ×RÛ?ßõ±Ï?Çþz"ù½? 2:Mïù?¦î¾‹}½?á3X®­àª?ÏÌ6pñ?ۓXæ?‹?Î@wðÎp£?Á}/ŽÈ?¢øˆ×€?âØ=Æ~£?³mã‹7?ѐîm¬?¯#ˋeó.?¨''!ŸžV?ž†L½øô?ëuêzÀÚ¾?´sâé?¸c™)Zã?­ØLJŽ4FGL J1758.5-3219?îÂÞjÀÀv–€àe0À:|r®sErÀ<
ÿ"Év@{Ý/E'Ü@
õ ¨ìô?ÕA[j	?îL%þpÛ@hò'hûl@Ñð~Ø£?ïÌù"@F¿àÓm›
à¿ÒjwØ~±·¿êìgpQ¢¿ïãh¬'Ä?íρ'¼±UNASNone	?º¼¯!ž?¶ãÐì%"´?½|0KL^?¸ðÝgñ˺?èøä'r ?Á3¦ˆö¬?ÆB¿¥"¹?ÄD‡NâkÒ?Ãaû À·.?Å=ä"08?å£ðgæm?Ép1D'ìL?ÔµQ0ߣ'?¯<ï)«P÷?ÒbŽA|÷Å?±Qþ|*™•?Øè £d¸?¯\ß@ýÔ?̔cÐEtÕ?°¦Ð0‹Š?Øù'=
â?ºä£•?ؼ¦ÚÏ:³?¶ÚpRù·÷4FGL J1758.7-4109?Ýԛ
ô«À õìløÀ9w)@k*À;´è·äÞ<@´ËLD&K@³|™®'?´ËÞæ)ë?ÄxÑ¢õbî@
Õ¥á¦x¥@–'(6*?Œa¢²¿Ô±d ·¿ä€¿B Ž€¿àø>•'ø¿ê«ïxÉ?¿ïòÔÔK4UNASNone3FGL J1758.8-4108?Î$£>3ʲ?¹'tFž\s?Âqe‹Œ‡?¸Xk`L?ãÚ}Í«ª1?ÀÁ÷$(ù8?ÓÝ°ƒ'¹7?È5Ør¤ED?Ɵ"G´û²?Â<8ÛB?àiF¬Qdx?Ë6ÞLÇûº?â·,êõ?®½¹'4–A?À>Ø(âÕn?£±«ÊùÃH?Ó¡%¿4¿^?©
s«í
?Ý»°³˜?£¾øm
­T?É+ÐÉ?£Òãæ?Õ®ÅD"áƒ?¦Ï]_•4FGL J1758.8-2326?ïø1q‰|?ÐÏÝMx"À9B£©½ÔÀ:"Õ¿º•"@ "»tৠ@Ö«ÃgÉ=?̕͜«qÞ?ÛG>©@åídòÈà?ûºouá\¿Üçòº•=¿ì½FA­?«ƒ¾ÆÎu¿á'§àÚ¿é¡!ƒ†Ý¿ïÿúÁҝÇUNASNone?¥Â'=ëz?¡¿Ö`PŠ?´¡' þØ?³n0 •?ì#¢Âm?¶ü\N–•I?žîê	lYÆ?¡G'Ÿµî¦?±+ʌlç?´:‹ø©ðl?ìã^'?µßôÅÆ-?ÀK"ñš²ý? zØG?U¯?˘:"ÁF\?¬¡œ||²?åbiª?® ŠÒD®?ŽösxåP?|‹ÊºúH»?©VÚM)–?šçZ¥Oô?íIÐ^?ž]÷Þ ¦Â4FGL J1759.0-0107?绘gÈï¦@&7ÏÃøõÀ9Û÷÷oÀ;c§¹íÍ@ó!6Ü`@ƒÂ‡çÀ?ÍÃք´?Äï@£3?òãII.?þ\ÀJ]qJ¿³G'±Ê½Ô¿æ‹¨ñf¿ë··¶ùҿ絟=Ø©¿ïÿòɶ—×?î*éŸ¡UNASNone?ëú€ƒ–×?´Èúì s?¤ïÖ	îÂß?£îù¤C÷«?µ´ãçÔ?±06ô1Å?é2ÀÖúµ<?Ɵ#N–'b?ªÞ€.jS©?´0†Þ0Øu?Ä}\˜z–#?ÂøJc>Ã?â=)֎u€?¯µw9·å?¶ùç"1;? …«ug_?ÕÇ2nÎ1?¬—ÐHY`?äQÈ$í?¶j6µ/G?¥ù@‹_w?'IÚ4ßÊN?ԝGÕD¹é?µ™[3ËJÈ4FGL J1759.2-0243?è¨~4í"@$¢hn~bÜÀ:cÒuðGÀ;ì†<Ń,@f°@O%'@Ó€™?Õól^MW?ïTów[0@ÀŸÀ$GÞ?ÿ=±nwí?îU€šÅÄ¿â;`"¾ŽF¿ãÝï3ÿáÍ¿ïH­M«"¿ïÿXJ?ïý÷ý}ÚUNASNone?ÌÞåTΨ?Ã6´y®X?ÍÞq&Çn?êŠTêÌè?áPªaz^?ÉÎBIøu?Ðršß+¡?ÏúØ~ÜÄg?àˆ.³¸¶?҇<©?ÌúEû^ÐF?ÆJZY4±?Ѽ*P¡7ñ?«ñ/Î÷F?×iàWÙ£?³3­pøx[?ÖÙõW…$ò?±š|Wè?¯ä"ìòÁ?›dx'–Ô×?ãa}JŽ?¾¬1DóëÓ?ÕASig«?»‡"¶QÝ4FGL J1759.6-1850¿ãÊo7#
@îÒ£¦bÖÀ9'ÿ#a.À:ãóbb˧@•o¨@Ö¥†6æF?Õ/š¢X/?áþ¡ñ@XÈh¹ý½@{èP¶Ñ¹¿é¶V˜í!?ïûáÝÖ	Œ¿æ!['—¿é¶ˆRIxð¿éÀ¤ ^¿®<kb›øçUNASNone?Ò:ªS?ÁÎõ¯©w?Øœ'"?É 6–‹ª‡?Õ±¹¦TàP?Ç>뛫?¸»*}ð­È?·s¶±eXZ?Ù3ÑÛðyÇ?Í(ù÷Ώ™?àN±ÂI­c?Ìïó[NM?Åz«ç"w? ï‰§‰›Ã?ÊÖÕæs'å?°
'%×
?ã럿iR©?±Ÿ^'èž?­i\ƒù^ô?"A}«â?Ò¨1™—SŽ?¸¹¹'?äÕQjôÀI?¸ÀTÚeå4FGL J1759.7-2354?î1Ƥ¦¿Åe¬­À8b¥)œ±À9™‡(}͋@ Ÿ:o°­@€ýÁ?ÎAN)Ø¢?΃*Ar>@€¦ƒŒçÚ?ûÞ?Þ½:3¿èÑÿ'›?çk<Žü‡¥¿Ö<×ÁóT÷¿áŽþµýþ¿êȸÀü4¿é–ƒ?4{UNASNone?sƒÕ¥Ò`?"¶'	•ìŒ? ¨T…,'%?°m65?îÎs'ñé?±škC÷u.?x*àcή?–3Mv¿ö?ÉN96šå?ȳ<krø?é.'üŠ?ÇÒ¢ß-"`?±~ɘ½¨1?'óɑYGN?Èÿ7Ž¨AY?¬"'Jò9ß?çXé>:¤?¬ÎM}ݓ?fÈ]½?WxAšCDÆ?«	3rFì?™ô"3©l?î9M}Ú?šTé.îH&4FGL J1759.8-1250¿ï¹ã¼Ó@5Ïò=À9¸Ÿb0wÀ;A;ʸ@ýz¤6@ÝâïN?ÉÌ7;*£m?̱8òÔõ@ùæ
‹t?õ©%Lj½?ïöBçÜÌ¿çÖòU'¿ãêÕ+@«¿Þ]¨[ý¿ìÓ~AÏX¿ïÿð懈öUNASNone?öóS!§ã?¶),òL,k?¥ƒñÛë»? F¼BN'ü?éºÌ×L?¸"7"&?2?ÁfG?%o?¹\x™P8?Ãð"ì[b?Àö¿2Î?æªhç"Ì?Àü6ÁM؈?Ô¨¹	œÌT?­Ì÷Ù¼?¿ÃÍÎZB?Ÿß¯LM'{?á³)ÁfQ—?­Ë_Óun?±X|³Â©-?"þô®™…?¾ý‰n J?£T$Õæ ?éõ@xYÖÑ?¨Eџ¡«•4FGL J1800.1-0323?Ø£m$×·@#•¯)M×#À9r•Q5}À;3Íw·Ò@Še¹ä@A#ßYw?Å¡«¡Y¢?Æ»Jî:Ü@8'¹ÑG†?özՖ´¿ï˜Ô!Õ½·?ëJþ€ù势è–ý»'"¿æªÑù\¿êLŠÝ"T¿ïÿö$´ë/UNASNone?ÒJÚßt¾ö?¬A |Ð?£ú¸A
—Þ?£"hµ€IÛ?åšç4Ç?ÃÿbÄëe=?ݗâIÂC1?Ëj¤fœ?ÒIgûËé?ȝ|n o?ж£Aðã?ĎÆi>Ë$?Ú%FÆ`B?¯`ïF£ì?¹ö²'}:Ð?œxI-¯¤?ßj.šQ
?­"'Âw	º?Ñõ*¥¡<?®+ô¤cÇ?ɓèìH	Ï?®GV±‡ó?à pr{n?µ¶Àüë4FGL J1800.2-2952?æ´þ«¯À	³åZbL%À:<†&öÀ;Ðכ\è8@ü±A%@Vî#^©Ú?Ò2B…Þ?éC´öl@©Ì1œZ>?ü°Rÿ?³«`Á`Ýæ?îtOȕ/¨¿áƒŠc›±¿ê0ô)2(q¿ìÀØ7d\¿Ý@*<•UNASNone3FGL J1800.0-2955?Óè|ïây?ƒBËS^Þã?ÑT±¿'´?ş'ø!^ð?æÞW~C>?ŸEQ÷uœ?­~EŬÏr?¬öWN"Ú?Ò
Ãjûap?È>üh 'Î?å"¹î''R?ÇZè?gzà?Džgc?¢%¢ÝwŽ™?Ö"OF4?²}Á^J?Þý_8*š?±e?{FpÙ?®'Ô/pNh?fÔ»ú'?äñäʤžð?³'3R(""?ÒIÛäȸU?±ƒe€ÌÜ^4FGL J1800.2-2403c?í""æE*¿Õ¾¤žvÀ9:G#«À:A>Ž±@"¾]ž@zÑî0Ë?Ð輁ûî#?¤8ût*b?çk;³´M?ü@°?è‡G½-óX?ëÍGF®Ê¿éö;ÏÆ|¿äûñþ_–é¿ãMÁÔÌ ¿ágÑ­ÝUNASNone1FGL J1800.5-2359c0?§«á3)Ë?}yŸAqn?["Q'"C‡?l¨lsÌ>Ó?ï³tOŠ?ûpz‰§?ö="óº?ªbKóÔZ*? û^XÙ?­›Lb†kõ?îË^òÕ?³ÂRò«-°?ºµ™èÿœ?›\Û|Tog?®m¼	?""f¿@Ã?ꌄ§|?¡Iî_زŽ?€þáßùaw?pÓlì<?ŽKáL\W?‰â«t» ?ïBÔôRé?Œ8siׂ·4FGL J1800.3-5237?Ô6"ñÀ,!ámmÁ¤À:óp–kðÀ<jm³aÁ¼@õ^£ylS?ó²õú:Ä?ÚsW%*ÜÍ?çZ)ûÒ@p¨ß‡ºt?ýÒv发X?ï«P°ò{³¿ìi¹Âƒó•¿"z±ÄU&o¿Ý#½¿"©@¿èW B•¦Æ¿ïÿ¬óéqHUNASNone?íÛgQa,b?°bë½ñ?çß«ÅO²?}^Öý?®LŽôtæ?¯§èôÖE?ëb@³ 5^?ăª@•"?‹ÎyãdÕ? µ~9àÓ¾?ÀeƒbB½ð?Æ­¿)jß?êøíCWeø?¥§à·òî¸?¡ío•PAô?ñšú:D?¿AÞœ¯J?¢ʨKhó?äžQEo®??¹äm~xaQ?Œuë^ȯ¨?"Ú¤Ž ¡&?Õß®*^?ºPY'XR4FGL J1800.5-2910?¿‰òwÀÀ`¾¼hÑ{À9"ùdŒÀ;æA@9
6u@¨âù3?бuBø";?Ԕ@~Ë7 @]›¡±–?û÷Zþÿ$?àɀ2Wk?ìùŽâ0Œ:¿áÑ>vˆH¿ëGÁ	Ë¿ßÛÄhû¿ïþ)›Ú¼zUNASNone?Å6{_Qr¯?µüqȼ¯ª?Àƒ¶ö¢»?¸¤ÙÂWãÃ?æ'sjƒ¦?ÀÏzíbÅ[?¶@§z›®?³Eÿ‡Zãš?µAð"Z?¶%ÍKbn?ê"éHn™_?»†LÁ–x×?Ĩì¾fD?¡º²¨1?Â;[+ÿ?¡Êõp) Ò?æoþùУj?©!´¤Y®-?­e–é€e›?Q£'"Õ?ɉá=Ã?µxÔkiÃg?çÇ.B'·ö?µ5fŠfe4FGL J1800.9-2407?íeÈm¯¿à]Ÿ¤u–À8DAYA»À9Îb뇢÷@ ì1"‡c·@Ĩm'K?ÂÓÝ7S(q?ÂÏڞF§"@
 ðbÔ
¯?úo·UlC?ïÿ&@±v¿ì§w¨®	"¿×
;&òˆ¿á¯`«;'¿æóû_‡O¿í¨]»WUNASNone?£)"'Ê?«å¶^²™¤?´h»ÍìMø?¼	ã#<?ì@OCÑ.D?ÁS9"ô¸?–œg÷¬§?Ÿ³ïí°&?¸/F9"Ô?»º'4ɨÜ?ìE3ù"ˆ(?¼–NS"?¸7&1?ž§f›—gi?»È­>‡¥ª?¤¿·8F|?鄣f,ƅ?©G¬Ï]?dûÐB
?U5p60Ž?¤…¨nAF«?'ŽsÓÊ?¨Ùê‰?'ØF@1Â4FGL J1801.0-2802¿é"	UÀº;<ìðYÀ:+PâÌÀ;¹ë1;â.@÷§kê4@Ôef—?Ìô¡}Ð<?ãÍ?ïXz@¢G²?ÿÝ#?_¿ÀçÉ'{Äò?﷙ÊAR¿Ýö5{âÏn¿ç5šìð¿ïâ&›u;ì?ê¯òkÂƺUNASNone?™RÛÖãã?'mQšðv?Ú°‰[³"?Époåš&´?â.ܛ?ÉKóh«C?´™¬ýü™×?µ;=õ
}?Ê}•~'dž?Æ	Go¹G?æÍe›Óž?Ǧ×~ÿô?À~£}lË?žG)kÞu?ٖÅñèmÓ?µCѬ-7?Þ*.¼XÛÉ?²ñ¿>;í?ÀIIÐZ?Ÿ'b:˜ù?ÛZcns?¶ÍEÍÇ7©?܁Ö©_}?¶7€g擳4FGL J1801.1-2626¿çE+øΪÀ¿û,0ªÂ¶ÉÀ:X`£®ÆRÀ<5ßüTz@ k\sÉPk@DR´Øº?ÒիÒ¼[?ïكÿÔa@þB҄?þ\×w¬	?îŠ<d4\ÿ?ÓÔ
c†7<?¶ûlâU°¿À]6fïMU¿ï€¤ ]Øù¿ïö-ƒÆÉ~UNASNone?òšë2Ž¦?äT`ù?äSÑ´šô³?É×ÚŽ:c?ÖI2èí°?ÉQQ¶Îdº?Ž~KczSÅ?˜^¨ÿv[Ö?áÀ–ê YÖ?Ñ­d¶–
U?ۊßУyµ?Ñ\6‰–Ö?Â4ôs'£;?£:m'áH?âÒh
"(?²áÎ:•Ñ?Ñ@µ±/,?­‹GšYÄí?zŠ`éôÒ?uZ$Tä9?íÅ«"'1?ª›ž²a–d?°*õP',?¨ùŒ£é™W4FGL J1801.4-4307¿ëµ!ÒJÀ#³y1DEªÀ:Tb(êÀ;ÛüwµCC@½±$¥¦Ã@œ˜D/ú?Ò§›ûH¶'?ÖáUðÍ]@UÆ2o?ýL…>õ?ïÿÕm…>™¿Û½?¼¥!¿å¤œâ¤O€¿èGGÝdI¬¿ïÿþÐñ?ïõv'[¸UNASNone?Ü?¦u'?ÇQ˜ùӁ?jR~²"?
'<bÏ?áb"è{<°?ÇH˔cí?ܬ"˜Qœ?Í "Öð\?¦½ïnºñÙ?¯Ç0)>,N?à†J÷È(?Íñ<ºÐžg?ߘýõƒ?°Œ7/¼4q?ÁVï»ÍÜ? 5¯ò÷‹?×»‹$_?­"b>üú	?ábsroh?¶W|¥Tÿz?¨¦{?"ü±»nÄ{?Ú9€Æ`qË?¶–W\0P4FGL J1801.6-2326?î°Tû¿Ô,™î˜ÏÀ6À.¬»µMÀ8óq}ñg@bQ#35â@IN…Ÿ?ºÍHÁºË?ÔiQÓ1jÜ@",pCß?ûøúJ3ß?¹Ëw7Dù¿çõYé€aº¿Ùk	ä/iû¿è\ƒ3&¿ê˜È]ý6L¿ïý ½é¨UNASNone0FGL J1801.6-2327?¯ö©ÓÎ	€?Æñ‹~'þæ?ã^™NÌ|l?ÑôÏwѐ?ÕCø'íEø?ÏGèˆý?uK,ÅÈs?‡f€¯?ä,ànÐ?Î;"ò²A?×P9÷EH¸?Íü8:w? Óö̔T?")h'ú|?à\ª†ð?·ÎílòÖÇ?ÝÔÇç:5–?·K	nÿM"?
áý–5H#?Î8ÍgãÖ?Ð]êÃo@®?µúÚòž5?çГRÔ?µúØþíÜ4FGL J1801.8-2358?ï€ä•Qœ'¿ãŠoŊ¹,À8''Œ6À9îC–Wź@!Í-Ŷ@e¦$ÂW(?¼"T=ïÐ?¢¨süüë?ñä¶Î]Ç@W``u?Áüža)?ê¶( Þ†¿äµešŽŒ¿åAÍÊùö¿ç™§ÜR{οݡ…Æ}þUNASNone?¥|`åe?©'"h¥Æ2?¨ÎÖÍäp?±
"㢺?í!:ݝb?¶²ö–@?¤¸¡Š*o?§‰h*ÕTm?­‰heÂC?µs¯
3wZ?ìÛß`«%5?¸ò+›Ej?´ëÆrZ®?˜Åê9§G?³Œ•-ù#?š©ëŒ0?êðô‹þH?£rêxyÄ? ¶ß~á?‹G™£`4?¨Bî<‡Ào?•EâŽø?ípc+öl
?šowזõh4FGL J1802.1-2652¿ì3¼'Úø"ÀÛšþôgÀ9Ë
By!TÀ;U
×ÊVÑ@ù
ö¸®ˆ@c4ÅÚjD?Ì/ú;É°?ãA³ß@ñ@ûÍxÄ6ü?ö"Gx¯p?í¡ƒræ§i?ï5+ÆWgÆ¿Ü2+`ÖÚm¿éNÜd…¿í/êß‹4¿ïÿa>ß8àUNASNone?•Xÿ#¾=	?Šªê<Mâ?â)Q´¹"Þ?È5ÞA}EŠ?ÚW̤Pòs?Ç·0
%R?œŽÇ`ðÒy?¢'òû–?ԙÁO€œs?Î ðMüà?äΩ8+3?ÍÄw7®?µiB'Ñ¥0?êe'YüY?ÖԚþéÉ?´ªÜK")Z?áèŠ;üv?´"~~À?rH
0;ž"?\µæÊw­~?çL,'¯?³|ÐÚ;JD?ц³1³L?³J=4K4FGL J1802.4+3634?ïé_c›c@9
TûÚ×RÀ;®ÉÀ¨ÒÀ=L-·É/‰@<# –x}@©Ã}˜²?Ô¶Òd'O?ëÄ=aŠ^"@£ñb®K@k
>pN¿ï Å®?ïýáý¶y¤¿×6ÿ[x³¿æ`¾ø¿ë)ZÖ¯O¿ïÿô!O…úUNASNone?Ö.¶5àŒç?ÍJ]'˜œ?ãRËs?ÍÞÏR…ÇÙ?©ia JA?§2FθÓ?Ñ+ÐxŒ>?ÇðS'år?ã¢Ä¨Ô§+?Êóxhë`?¾=Çwx•ª?±c!Â<¾?Ú´\²È‹-?µ£Qyü»6?Ùb=çs.´?·}=9εu?ÇÒÊˈŒ??¥}ÞÅwž?Ò¯µ×‰HÍ?²p¸ä(ë?äþ
C;?µjF—Ú¥?ª¡'œ? œ¹®ðy'4FGL J1802.4-3041?îQurÀ3YÀ+"¼ÃjMÀ9¢{oâæëÀ;ÍÑÑ‹è@dÓr®HR?üېIŽ¿K?À¡u´6S?Ö
´ôhó	@åB˜I@†â8™Ït?ﯦ¶¸ŽQ¿åé,êCÖ¿Öl^"9¬¿Óoô¤Ø$¿åÚpú>¿ë©ØÁw¯UNASNone3FGL J1802.4-3043?ØÒ¦ØÑ4R?À
ÀÉӋ?ӝ9mœS?ÁW+ Oå?Ӑ–Á/\?»"è¤
?ÂpJ¢']Î?¿L¿èùžÌ?ÈÄ<ÅjŠE?ÅI_ù5t?å2Þ&…ü?Æ´+þºš´?ÔÁâÐh?÷?¯¾ìÿ*5×?ÙUéɸex?²ÄùDD6[?Ñè3eßZ?««Ì2?ÓcŽ (>Z?¨TÅ».>\?Çh½jšî3?ª Ðz?àt	•E%G?°à°G‹34FGL J1803.1-2724¿ïÄ5a`ÃÀw_}>@À9m@wÏDÀ;÷¹à`þ@4úXKE¤@·Í+d2?Äé‡B©ó¯?ÐTÚ¢ÎL@Jd`Ò©@\+ž>nü?ßeˆÜ?Çõlh³ó¿ç'•`$¿çÁý &¼¿ã.ÕÖ`ÊE¿ïÿöàœjUNASNone3FGL J1803.1-2728?Á``Ä=§?³}WfKTã?½a{sC‹?³Û­ý{ÐÉ?è[Ÿ'-Í?½à´eöƒ?¾[O:üN?µ	ˆX‡ao?¨I旗¡Ð?«-nn#h?ê¯÷¯FfY?¹bo»ÕWÎ?ÉÕÉ>f/?¦N"Š3Éí?Á'q7"Ù? 3x"Á½}?åIí?¨íÛa"'?¼™8ǖ"‹?›mÅ®î?¹ºÿ@¤ø?ŸàhwhBÎ?é5y…ð?¥h~Y¶êñ4FGL J1803.1-6708?ïÉsø†u6À4[çÈіÀ:èÅPØÀ<Rdë<#@ü:à>Å?þ߸Í;‡–?º†ÕFÃÞ½?Ð,âxY@|¶"‹ë[@à[8Šàï¿æË£¢1пۮ!æڕ¿ÝW˝>?¿à./ˆƒÇ ¿êÜV|E¿ïÿÿ&¦³UNASNone3FGL J1803.3-6706?ëè?Sáx‡?µŸop?»ÌÒ4Cx?´&×5åÝü?"Çò:ÿáN?V3Å?ìo]¿¥?¼²F5'.?¦‹ôbe?µÆ}ãe®?±A[wñª?­¯†nÝ©?átZ^d?¸ÂÌ}¹?Ö4dÅ3¡N?µÕÌ¿?¾ªÊ¦‡¦?¡Œ¤5?ë¹{è"?œ8ñ~	â?¤{MCB,?Ë®ÂÕ?·özNé?•Äøº¡œE4FGL J1803.3+2425?ïHi"lƒâ@4ðx…LÛ{À:SºÜ	€²À<
A¢a¿@#úVå@¾"[Có?Òñý=­àx?ä㼝ª R@™Ê&)_u@¢+'ôØ¿àí0_nO"¿æߝ‰é"¿ìùXç!â©¿äŒpPÊó¯¿ï½þž0§¿ïéÜ»WUNASNone?èZÚáCWª?ē•OC…°?Ëü]ÐY^?Ä4^[bÝ?"Á»q?×?—"dzV?Úÿh¹Á>R?͙¸Ý&wò?ÜâHº¦É?ÏF£ŒVï?À</ñD?´0þˆg¹™?âÄ=³y‡'?°ÌŽ¯@|?ÄJßX£ë9?¤OØÁ d?ÐRìºü?ªžíNŸ@a?ßrɈì
ž?ºòÁw.å?×uÅÑõŠ­?½jŸm¦?Â.áJ<Õj?§¡Ð-&¹!4FGL J1803.5-1639?ïÇ_=äMX@,ئãÀ:"¿Z'ÈÀ;ß[.ú¿N@zƒEÅ1"?þ­<^Uí?ÙÓ»¾Ýuç?ïBR‡"Ä@¥b?8È?õ£Þ&;~?ïí(Œç°¿ç|˜×ÒºM¿à±Èà5j¿î'á@øÔ¿ïÿÅGMƒ?íaâ"oUNASNone	?Ózü6[,9?̾‹T﷜?—Õ:¿™%?¦ÔO`'äœ?åƒØÙÅ?ÍëhI2Á?Çwć&4æ?ÌêAûÍ
"?Ó}á[ÙÇ?ÑÁ°Äº£?à—Ï툅ã?ÐãŸU¿U?ә6ÃNȼ?ª™Ò<Ä}?ÒW~ˆòU\?­÷ó†ÆY2?ÚJ³¾áæ?¬äÐ¡ºt?ÀöCÓ¯F?­'uº£ç?ÒzA?Нñ?Ã
–"Ët?â…^O"Å6?ÂÚ"œÐ•24FGL J1803.7-3207?ÞÍ[Á–ÀâP.ì|•À:
5Ä+mÀ;ó`µL~@ŠŸþ…,@ù×Vé?ÌÍ£6{g?Üp¼`mþá@;=ïí™@ó
Ýԇ¿°žaÕ]-?—B&rþ¿æÛÆ/#Ùú¿åÚv»œ#¿ïü`Ÿ±?ïÖ¢
±nUNASNone?¶¨³ŸVe?¯øÓø×g¾?²ÎôÆÑi/?¬Â¢ÈÝðÎ?êÑ
ó;'?¸¹µïø ?ÔÓûȃõ??ÈòØï‡0;?°4~Üÿ–?±Ò£²s¢$?㏂âen?ÉË!¡½§?ÑeFq¢/?­‰(b~ç?Ç_¹4ëäÙ?§­¿¶Ä;?á¢_Œ5²?°aÃ$Ð&?à^ˆ‰òd?´VZc}wî?·†TóFM?žôWÇxue?ÙbuÙ¯I¦?´8eÉâ{
4FGL J1803.8-2908¿Ðm…òü?	À[
Ø/×^À9··ä|À;UûKeY @X4Pi¥@(©6Ŏë?ÏLáÚûä'?íÕ€ÙÚ@Uí¡Xª¼@¢ŸÒ™?çˆ]‡º¿Á":šZ´¬¿èœRnM¿ìz¨<ʋª¿ïÿ¹ô'ô<¿ÞՋ¸/‡UNASNone?²@÷Hf?¨dѶ-áÜ?äK$¶k»¯?È[éz
?ÒÙx˖ƒH?Æ߬G$c¼?©à"¡,éè?±ŽÅ©¢%?܋	j¶ýe?Ð5¸Ù®?àr'²¯?Î ŒA¯qr?Ê5ùZöC?ªK2–	HJ?ÖQOÑUjF?±{÷š{yŸ?ܓ³/t1?±¡Gä+ö?t'ÁEy–?bS"éoΜ?écwÜ>8	?±9ˆÕGe&?ÉÐèüô?°év›çAÖ4FGL J1804.0-1124?­r/ûQ@r€Æ^À:)vþUÀ;ÇáR•Ï
@D•pÀ–@Ê)"]È2?Ñޘ\Þ|?èd÷eýŠÛ@•—'$@8 GÉa?ï69bwCƒ¿Þv¦…:g¿å
¾"Š"¿îp;Ñg¿ð?ïÿþˆ0»ŠUNASNone?Ýõ4ntLÖ?ÌG>rÍØ?À孚d¶)?½\oÀ«?ٗôÄYX?Ê1ë@û?Í°Ì`kD?ÆøNnU§?Ò{øBw?É?QüBɞ?Þ¬'>Ò.g?ÊBó¸Í¨?Õé‡/²'»?¯mùÁ/XÏ?Џ.IÎÔr?¯m7¼pò8?هJ†~˜Ó?¯i&¯5à0?ÉJ¯òŽ_š?«,ÛwjB'?Õì"Ú\ŸN?·BÅëHY?Ýn…,\0å?µSðC–Ÿ4FGL J1804.4-0852?æú_]Yó@ò[1~þ
À8ùg+ˆDÀ;	q(aH@~öº†ú@¼R?¼©HðÕ?ÁØQeMa³@›ð™Z¯y?ÿªñ=D"¿×
P`½§¿ápv̗¿èÆ6°–5¿à½!=èBõ¿éþ=½Ð°‡¿ïýtÀc‰UNASNone3FGL J1804.5-0850?ÚC¸·~>ô?Á#Ï E?ý?Æ´*:Žº?¼kÿlHZ'?Ú¶m3dy°?‹@k7l??Ã÷3ÃíòÙ?½¯«ò౅?Іø®5s?ÉQÍLD?â¾·­h?È(˜_MTc?Ö¼½Ú9«x?±Uf­"4`?¼—rH2?¡°z'?á±$š'ž?°êëÁu?Éñ~ÏyÓ?¥ÌÍÎ=h?ÄÖÙöWV¾?¦¸Uí?äMé΋å[?®ª…ðk'4FGL J1804.9-1745?èâÎfT%?ýjJ÷uÀ8ñOýnUHÀ:¥}§Ë‹"@© u@t@ë:Æ¥k_?Æׄ¶³…Ô?È#ë†Lá@›´&Ú@š€©•?è°×£Àd	¿Üúû´@å¿è·—{ž¿æÀҝòâ¿ïátYn0_¿ïʓ׸¹UNASNone?Äg–ëWš?¶mºOÎÏ°?ÀvŸÊ£Àÿ?·ó>3šƒ?æÝþ'œ9Ú?Á®'@˜Ì?Ť3E›ã?¨PU"bS?ÅEi´]?Á}³Î¯f˜?åE˜èÓÏ°?È°òÔäS'?dz–gËg¯?¦D0³–/v?ÂGô`†)?¡ð¸°h`?åM܄Š?«íðVü¥?·Ón¶¿5K?š"˜ãÚg?¾ûPKÓTh?¢o2½ïíð?é&(­®Ê?¨‹µ#ÚX4FGL J1804.9-3001?Øk.Æ«ºGÀ½–ÁxôÀ:NBM'iÒÀ;Äq£±J@š&\`(@
r¡Þ¹?ÒËáÀNå?é¡Xª¼Í@XØ>?õ5ßðëåí?éŸåŽ?Š*©_Ù¿â©}g^ß¿ëY‡ZÒ´m¿ïíVy-?ìÐý³õeUNASNone	?­,¢ 2>?¥øáü²~?Ë(K|Á?Ã2äµ?çc"ÿ]•›?Ä- «?¦ö?·/h>—(?º¹o÷²?Ѓê^MŠà?ËÃâlVh˜?äØɇ«?Êœ[.ß?Æ·¸Ëß\?£Aþrÿ?×*P=¼>Ö?²ÿ+|´?ÝyÓ\»Q}?±eK­Ê:8?•U³Í'?~µ•O¾yú?å;Áê?¤?·-,5'J\?Ô4?Y߀?¶b@û™4É4FGL J1805.1-3618¿é;Ëfß÷¼ÀóÜìՁÀ:wè]À<Rµðè5@VðqB8?üç,å;Xœ?Äôe˜
Ma?çuÜ%/dr@Ÿñ=Å]m?ù·Ÿ•g¿ïøI©ƒò?ïÿߞ¶Žó¿¾í¼[t'¿ã؃ÿÿT4¿ïÿþR€ÖT¿ÞÛ^ºËmUNASNone?¦À-Ϙ2{?¯±3vÃAŸ?êuT²15?Àfi:æ?À{×9Q.?¼le&ý©É?—acÕðš?¡ŸØ-üµ?çr…µp?È´¦´¢Ç?ÏKÅO+(q?Ǧ[8õ?±vh‰Õ?—`".}ªJ?é]eŠõwx?§Œf6'A?Áÿg˜õÝ4?¡ÔQÀG^ž?¨R"nµ¢º?š‹`mÜÊ?éIËI¨p–?±Ž>Ֆ?ÄÄJ=°Ôþ?® ¿» Þ4FGL J1805.7+3401¿ç69±bÊ6@7ª>iƒQÀ:A8æÑZÑÀ<?¨Ï—'h@p4Æ[D@…6…Î
º?¿m´¹Zª?Ó\K$Á€h@ûd8Š‹@óΆ‹Iö¿Ó˜dMk¿Óɏ*ªÎu¿ç
´¾¹
Ó¿è¬.È—‰¿ïüVB+ô{¿ïÿX°›>UNASNone3FGL J1805.9+3407?à
£_*ù?ÅöO'…å³?Û‹šˆO?Æs>h¾u8?³Œ¸ä>1?ªÈ~{‡?Þ\-¥+ã¬?ÈïLSAá?ØHGLlwÏ?ÈÏ	úç×?·ÏI?²¤e$*¶?ÞxÉfº?´4ò³h?Ó³{ú0½?±ó\qà?͝§u?q?¨~ÑkmMŒ?ßüæ6C?«}¨Ru¦ä?Ò²2@ÂÒú?®?…až‰?Ê¡Î`3†?¥KÛ"HRC4FGL J1806.1-3344?ïÕ
_RåšÀÌ$·omÀ:KX+:@nÀ;©$7í­@*RÁ@|¦CÌ?Ë÷Ám9Í?ºÛ~K››?ôC‰!|QŠ?ü
zW_?ïè³}pn'¿¶1NA+™a¿ê-uïpeÄ¿Üú"[ADC¿ç©E©W|¿¿çh̽]nUNASNone?×.}8u›D?Á#%·=Œ'?rï//#Eü?kG.féÙ?äBãfëÓ?Á3ü‰€ó[?ÕE Ørê?Ã(ªHhe.?…CYK¡À?—]ŒµOý?åb—e?‰?ÃYýiúbá?ÞE3"EÚX?²"‹'tôð?¦i²eP³?‹ÆǼ?ÞêßEm{'?±W¾}óÒä?ÝÓlätR¬?­†é±Áã9?«6'¨×"{?"â>¼Š¾?ÞÅÎ&pÉ?­mR¿§Ó4FGL J1806.2-1347¿ïV'Iµšp@ͨ_/:€À9d
`:Ó;À:¦R©@@P€u[KÖ@<ÿ?æ"&À´½?Ú|ûî"ˆ@Ô²ÄãÊ?@Jîí^Ù?Ý·äx:#¿Ì"è^x±¿ëêQBóH¿éªÞe{…¿éipafø2¿ïãý5Jd¨UNASNone?ÒK'¡h&+?Ãd•@Y?ш`mhšÕ?Ì'èU)a?Ü,ñ/??Ë‹.·ê9?Á½¯¤×ì?ÀÌîÙþ?ÓGyuÏç£?Í¿Hö¢¨c?áíÙ.Ö3?Ì1y]¯Ú?Ë¡¯ä˜9R?¥ëðÚn+Ø?ËNèNo¯??±°¡JÂ+¹?âCÙó>Û?³
ܙq×?©ŽdâÏ?œù'L?½bíAŒZ?½Àˆ[µµ?꺼ÐQ%?¿àWÉ}~š4FGL J1806.2-2126¿ê†–?›¿Ð)TÂÏóÉÀ7œ;
˜	wÀ9{ÛàfÅ@øùSéa-@¯R¹
x)?¹nV\ƒ?ÔfÏ­QÝB@œýÒ(V@‹Ù_'F—¿ëÀ³ï†59?äɂ—½¿çEfîVŠ¿æ;_ýk¦¿îCC¡•f"¿êÕ!Ð4`ZUNASNone?jƒË~Ç ?bã'f(?ɗ'³ßÜH?ÄMAåêˆ?é€<Š'?ĐySxQ?€"£3TnQ?ƒÃ-'/ކ?áXµ‹=?Ê}é¢É˜?ܲ{O*?Ê[s+Âç?¤§â41‹?"'Ù™¤éþ?Ýþ"~eæ?·G´œæ·?ßlp:ÜyI?·)®:è?RØèaë(9?FM[ÒÐo?Á±©JYV‡?¯_©$ï?ëŠ)98´Ë?¯.Άš4FGL J1806.9-2824¿î3,ÖÂÀQ1eәpÀ9×]	ÆR_À;i²lÏ64@ãÂh@>±Ä2ÊX?ɺwàŒGL?Æ"³‰.èK?ÿ9MÿgSÌ?þÒ&"©x4?ïøò?Mé¿â›`
†Ñ@¿éÖJêà¿æá@øÔ2¿æp,XN¿äiUßZ˜þUNASNone?Á#Wý6ÁÇ?²ùn˜LzŠ?…³û
…Ñ?ãÔO 8?ë`Z}Ùw?³ˆÿƒÈ¶?Çî\åB?»ïð%7ˆD?"
Þ韙?™ä*ãH?écùÏmEË?¼^mÙ5¤ã?ÔTþI!–w?®'™*°ù?°sRé?Ž¹S‡¡ß?ãÇ Q+dÇ?­ƒÕw^·×?ÉA" úŸ˜? ù2:ð7Î?¯"–ruhs?"%ÌÌÐ#?ç¶Uš"?£rÿL4FGL J1808.1-1234¿Ým4Á0j@
7S½vÀ9—žþ]h'À; Y}I׺@9 M'Úä@A*¢jùs?Ëub'¬K?à™Ã‹«@çԝ{¦j@Xbz¥c¿ãæ5‰NÈ»¿ÕÉ^BÖiY¿å¸ßDž•'¿é"+Þ«¢¿ïwj·-ÿ¿ïÍî'Ò-UNASNone	?˜\"E
\¶?"!'nU?ÆS«£kï?¿ÐðQ¿Œ?é¨0ôü™T?¿÷XØ̯?´'Û÷Á	?±bæà…Uý?Öâ½+Ä(–?ÈbKÀž¿?áüeë<S"?ÆêB4‹^ú?¾,c2»h?˜Áõ«š?ÎY"S?­¶ùŽ1?ä·kýYƒ~?°RÁÚl?§úßlx—^?Št஍Ÿ?Ì!æâ×»Û?ªlqÇv?çwØP'‡"?«Áa"q4FGL J1808.2-2028e¿ì¯ÐÉl×*¿ÇN%ýÀŠŸÀ7»èc+HƒÀ9 »åô»ÿ@'p0?@Z"{$c?ŋ-ۅwN?àQµSGP@D¼­šØ^?íå¢^±‰?ïßï¿@P¿àö¨ž[¿àŠN½Ó4Æ¿êd†'UØ¿ð?ïõò`L–UNASNone3FGL J1809.2-2016c?¥×/QÉÙ)?Á5á:Œ¸? M£Æó?¬>àN_?흲Ù7Ï?‹PÑ@Oæ?'}?âø?¡Ô~åX©œ?Ûl½÷xLo?Ñ+‰5ÛÙJ?á½·,ˆ?Ð÷Ôª\X?²éÁ¼"<O?žàܸ»?ׅw©©.›?±-ß1¥y?áàó˜á)?±HÀsû!"?6j†PaÙº?0œŸXP¨?Çk'+Ìõá?¾"ŠEJ?ê"häB¶L?¾—'c4FGL J1808.2-1055?ê•ö–—(@¿ÂÀð À9 Ô ~$ÉÀ;"ËêN½Ó@¸Á'Z@@ÀA¤>?Ò;"ÀÊ5?éXV£zÃë@"XýÈ[@ëLk'?ïÅbu@ý¿jØ»dç؎¿éÍd1Xh¿ìõºAYç}¿ïÿÿÊPË?ïþÍeyUNASNone?Éξ=?À($K#c?ÊÄyqJÏ?Ä?œõw–?âÛaTI‹?Ȝڝ#f?Ʀ4Ñ˵¾?Æ8Q¤èž?ÙøŽ|õHâ?ÍrõjM?Ú´W$Ü??Ë$.¤Ýٓ?Ñndq]®i?­ítŠó8b?̒`¤{?­"Màj?à$F/ ­?±äúÜjc?´4c/ÃîŽ?œ%ÿUù"ß?Ø´ŒLÀÀ??¼#s
?á-s§"?»g0Y"ˆ'4FGL J1808.2-3005?º Ïi›`Àd¤L{ÖÀ9âOOÉkïÀ;oÑEØQe@« ¸qÌ@É$¡ŸøX?̀–Rè/?ÑD¼@àÛwŠ{@žªfpwa¿å¶PôåË?ïø曪ëѿ僲ýmÔo¿äØ=‹ü£¿ë©n*¿ïï¢OJÀîUNASNone?»:ôŽ/¾×?¯¢âýÍ/?­Ëô3?¦±¾q®y?ê»èŽñƒ?µÍ>`´é?Ó'3Dã!?Â=½ OíÀ?ž™¿'w;? ¢HA"e3?åw˜aáԘ?§ùWoÏL?Îò÷½u~?¬sü¶´¢?Á>"áŁ?Ÿqg›?ä2óœØ1A?­ä"¸f¦¸?ÜÒfÂíÀZ?¨¯ã€õBÇ?¸}Ü@"?šÅY‡iÎ?Ý-—]›/?©/ç5Bº 4FGL J1808.4-3358?ïÚ;,HTÐÀæØnÁ~»À9…ëOnÓÀ;ÙJr'@pޚՃÖ@Íþu¼D¿?ÀN¢dïBî?éV؉™qV@#4h‡¨ÖM@ð™/¼[;?ïõÞs¾=¾?Èz Ûmé¿àEæÉÎË¿êøToÃÝ:¿ïÿ¥'(^?îK]@ÍЃUNASNone3FGL J1808.3-3357?'äѕV¥¾?• ¹áù˜?íÁ‡ÛÒ#?¸b}=ãù?³X¿[ËÅz?µŸZ6ä?Ž±ƒÂ!‡Á?šôÇŸ´â?êI©©Iƒ?ÂL:'P?ÄîA·ÛR?Á(¢ÝŸ¸?­,~Cëðm?—»íS®?èí¹Å3+7?ªKÐ|÷¥u?ÄýùZ8W?¥°Â†)†?oÌnŸNÙÐ?a4é҃Æ?íÔÕÚvï?Ÿg"Z›
?°Zí·QyÃ?žCð¦zÕ4FGL J1808.4-4521¿ãûØ°¶8À'úƒBØÃÀ:>ýž%ðUÀ;ëø§F*‡@Öáü3í˜@á՚ѧþ?Í»{Ep¢?³š¾‡ºŸ?æ^æªÄdH?ÿ –˜³?³?¡6ÿ½Ý=*¿é†väÝ¿ã@+~³å¿à)¡N™Á¿ïúîéWG¿î?™UNASNone?ëˆ6öçÞh?¹
TŠ5ï0?ƒ|K×}¨"?ƒOžmÙF?À§_fè«Ö?¸yõ "L
?ë¡Q<£$Ï?Á™h¦à?r£Ypôå?€=-=Ýâì?Àå AëÌ?ÁbÝ>¢læ?ç­¦«
Ñ?°2j`B!¿?©Œ@>
f?"6"Df¡Œ?Ë"ÙDE_?¬‹{å!SA?ê©
¹\Úã?£|#™Y"?ÑHºú?{ÈRûÂqÓ?ÃA¨Jc}?£Ë·Ùf4FGL J1808.4-3522?Ï$][¿ˆ/À•–\Î70À:ôj{žÜÏÀ<aÏ'ðà@@W¸"Ç?ú«»Š…) ?Òt¡ýì)‰?èÓ €étx@
†ݒî@g*÷O'I?ïù'áê@P¿íßRáNd?ÝÊ®›¤6¿æÄ}ÈØ¡¿ì•à<Z¿Ö×¹ºÌD<UNASNone3FGL J1808.4-3519?Ñ+~ÉN¦š?Ɓá?¥áÇ?¦†f->É?£€ž|žÞ?æÚ8‡èÇ?ÇÊf#ax¨?Ý\S´n!?Î.:Œ©? *Tór!?¯
Ž #Š?àO0ÖÇAÎ?Í¿Bütò?äÀºŒOÖÅ?±ÆëÑeÒ?¾‡sm¹4'?¤ý')?͹\ä
Ù?«)º7sJn?è՚¡ß²É?®;…çqØ?¢ö¿Bݒš?•ß›ÿÝ!K?Çëå§ÉÐ9?­¨£sŽ}]4FGL J1808.5-3701¿î!hÁ›§wÀ \¥ß"9çÀ:%а‡éÀ<Ö¿•@raÆn@«ñ'l?Äær$àŠ?ÞÿÛlø§@'c/@ñÑHÝi}?難¥¦V¿´'¸N»yé¿âÁ' ÿT	¿çaÃ3ÆÖê¿êYè©¢%Y¿ïþÏ´ÙéUNASNone3FGL J1808.4-3703?Ÿ_9&Ìa¬?¡:µ]€?àúªT{ò?LjªÕØC?Ü	êB?ÆlĪÄÉô?Älió˜ á?Á>Ž	ùtX?ѽÜòá£)?Èá|O`ß?â÷	©&3?ËÚ£i`ñ?ÉgZ²qŽH?©uÇ˜?Þë½?³˜âÐx?ÔaQ–¾{Å?­ÌA{Ÿ8?ÊÁŽ[!p?£Žì"(?ÚI*a£w}?±ŽWöó?ØV'.÷Ì?¬Ëp¨ÌLÈ4FGL J1809.0-2853¿ë¤•µx66À­Š—ž×À:]xFÜ]À;އ$L£@v ís`@è«ÕÜ@?ÒíýÐ?梐MÀ}3@ÃèPïÝ@%&¹Óø?î)<7B·¿Ô€ûþh¦2¿à°ž~蝿æ¢CŒFÊÀ¿ïÿÿ)@k*?ìôí²öaòUNASNone	?ª5ÁuU!Y?¢)y''e?ÕþuìK?ÉÂ1ȱ©|?ã]\.·Æ?ɆhRðÓþ?Á¯¼àι)?¿1oðÈÓ?¾tîƒ1‡?À®Y°ÆU?çŎ©ûë…?ħ'¤†Gó?ǚָ!P?¥Ô4Íâ?Û‰ŒÊ
?´ÄDµ"^?Ùö\L?±WÚ\ûQ1?Á©Rþcâ?£mÉ/‹¿?Ñ
,)?µC¸¿Û7?ã	&uªs?µß
àý4FGL J1809.2-2726¿çMÖªœ ]ÀÞ9ܚ À9"©³`ëÀ;32¯È@ÕÜÔVÙÖ@w¶ :‹?ЛB;8æ&?Ê扷N``@
Y*f—@MŒ£ ?ïûÏ^¢wº¿ÙEíÊ»{¿è"d~.Ú¿ä-œ»	h¿ås°Á©X)¿ïÿýawUNASNone3FGL J1809.2-2725?Õ®evLý?Â"ô‡Â]4?©öö7Á'Y?£ÁìÂÑ]ê?ã‰]á]iT?›>v#\?«zÊ£ò/?¸¤ïH_?¤_¨òxì?§vÍVЉË?ê&¾5ûå?»\L"þ?Ó1ˆ@çdç?«_}à"Œ?»^Í»]?šø±¡'?ã°Ôہ?¬3'œl&?À¥I²^4?š_¨½»?±)ê·_å?˜mR=QI?é³hV"<w? ¶	Õ°Í4FGL J1809.5-0816¿Ô·YÌ,Çg@¥ÊÞ¶]À9gÙÛ©¢À:ì™+µ@Ꮐ[@ôØý\·'?×T=ø´?âÙ`.@÷ñ"íjÒ?úe–w¦)Ë¿·ZŒhƒ¢?ß:…\ '¿êž`lQb¿ëÜÅ}Î¿æÈ|`x»©?ÈäD˜`_UNASNone?ÉTC/ >?¼¹NÅÇçþ?ÁÁøç
´?¾dñïô¨é?å:pútƒW?ÅA\Wæý?Á÷»¤v#ž?À⭉ü4?ØÚ ›"Cé?˽S(ݘï?Þ*'0ªF?Êf­rJ¡?ÍL¾9¶œ?¨·ê°¾v¬?ʆ"ø•T?²–Ít4·@?â+ksm?´KŸBgä?³4r%SjÛ?˜B?ߏ¿¶?ѓ[bŠv?¹Ú̗áz¼?äÏÄ
"é?¹di˜Ú84FGL J1809.8-2408c?ê×<$H‰²ÀDÍt'yÀ9$«Ô.ÁÀ:{Åyò4e@;€3ìì@>üå™Lm?Ñë>|è]ø?ã¤WB‡'@d>mùÙ?ýƒåîy¿ÛO[²Ù1¿à¾Ûrþ¿çŸTžè¸ç¿ëXÚϐ¿ïô…¾Eu€¿ïüø^KòUNASNone8?ŚƳÔ$¹?º2ÝŠÁ£?Ç'6J±ð?ÀËì,>ÍK?äπÀ^¶–?Æ(Fç'…H?®"v<?¯µ ²#cU?Ê5Ñq(xU?ÅBê¬b‹å?çi±î~)?Ĥ!/¤«e?ÁeQr9?¢5ï
¦% ?Ê@ú¸©j?¨Èçqÿ:Ÿ?åŒ=¹?¯2q	‹?|v=º¢&p?fc'B—o?Ìs=sGFý?°¢5®{??èªD'¸éô?°±Ê.…²4FGL J1810.2-3054?âšÝ[1ÌMÀfù3]$žÀ:{ç¨ñ%rÀ<	0pá¬@g0{óÁX@D'¾‹Áj?Òٛ\'R(?ë¬<Ԝ¤ç@Ñ÷ÿ€~@@ŽFø7	?ï÷`‰­"L¿á1;A®A¿µù3¡ÜÍæ¿îÇ[¾í'¿¶",maZ¿ïÿѧ' ÖUNASNone?Ó^ûJU?Æ;|ÜNšâ?·4S¿¢˜?µ7Ç,Ëg¼?ãžI÷âá ?Çß1s\4Š?К¶F•Md?Ç'SÚ(ý	?®¨ß9fõ?¶ Âu§?åÈé'ß?ÇÿSu+ùC?Û¥(æŒN?­e#œ€ØÊ?Ëöb·m¢?¬÷L•¤?×){bçá?«H'3IIõ?Ù-ÛjR?·Bºo'Âã?¿5Ԙ5?³à¿qÁã?߯o @-?º‡DQÔÕ4FGL J1810.3+1332¿ï`_4ݜ@.A•övêÀ:eÜyhÀ<¤~Ïé¸@iÑãâèî@k;¸<òÐ?È÷èÔë?Éٕ2+Ì7?ÿ¡Ž«)?ù½X›L¢? Õ`¿â4Šˆ×¿âÚìJ@•ò¿æ¦]—ŠË ¿ì¬…dXo-¿ïÿø¨ó©°UNASNone?âXaþ[®s?Ãõ]@už?²V{2?«;q'Ý?ÖÇumÇO?ÃçåõO?ãé*ÝÖlÃ?ÊïçZŽj?ÀœÝia§-?¿%âȅ[?ϾwD¥È?ÅYœkª]?çâ†9t'r?«;} Þf?µ.´Eq·? Ò½Ú?ÅÞåÀ
ý^?£w\îx'›?ÚÞÝI‡âß?§mLüAû-?Äq˜epL}?£"ÚñúM?ÚèVƒ¿öã?¨Þ'ÍœU4FGL J1810.4+1700?ïñî…ëM'@0ŽÓǒÑ(À:l0 ±»ÏÀ;ÇVpOu@™¾JÓãÂ@Þ?©c;?Ñ8š{@èþ?ÒþÄt¹@b¼ºh?ú[oó¯¿ï¢36ÌE?ç†tX—pÊ¿äÜþޗÐl¿éÌ«ßí;¿ï°ÿ笿ï^­À1ËUNASNone?ã»â|}Y?Å^BHD?¬qQÙ¼yw?§ãŽÜ½!Ä?ÔúÌÁv ?Ä°ˆX¶:%?åÿ®ëé)?Ç]XÌÕIœ?È#û	8^?ŨÁoj?à;;"û?¶D|1?àV	–½
~?°é'Œ‰A?ÂÁœ8á}Õ?¢™3קi£?Õó¶&?­KÂkð?Ùî"J¿¹}?®7·"5¤N?ÈürÅ(¢­?°Á! ?'h?ٓ2R«õ,?±ARJªÄ4FGL J1810.5-1415¿ïÎTgÇu±@·|ˆçš®À9(ê°£À:ˆ¿™Þb÷@ÕÒmrÊ@ìbÿ©˜ë?ÐÁ˜ÜZ^p?Íîryo,´?üQ*"ÿ&?ñ?ƒxšñ]?ïb´•žbV¿çWy-éGW¿ë:§0[Ÿ¿å+,Ôt`û¿ïÿü¿ÙŸC?ïÿÊjåQUNASNone?åÎ4œä§u?Ç@ÁN"?¾+ù¹‹?½5¢fЬ?ɱ0¯ä«?ĉZõSŸ?Åm"??»?ÅMûÂó‡?ÇjgîRþn?ÈG÷PN:?ä݊»Ûpv?Ëæ€&+J?Î×Vm)À
?©vÉèm€n?Æ/½%ÂC¦?©(0R?â¾;Dÿ?¯ꁰ†c?'lˆ6â`?Pû87ì3?·G'¤Š?¥wš'˜"?샹YT^'?¦Å€«Ÿt4FGL J1810.8-3347?î'm¿²CÀVAb ßÀ:<piõg À;¾9ìN@ád^y]@|ªu‰ð?ςe"oä?Íöc7‡×@œd…D@³jÑ?¿¸v×LØuÍ?îx`äÇ?¿äxrØd°"¿á,|Ë,¹œ¿ãúÍ[h£¿ïü½Í«oUNASNone?áƒýžß"^?Âl–×R"b?˜Ìë1}v'?''œ\þž?Ûk6(ÿÛ?ÂPKÝã¾?âFL:­@¼?ÈrÓö‡ij?"Õzh¢I?‡)v¼lX?ÚÌ»·d'u?È#Hd/څ?௢
8L3?°3´Îâ1?³Fs8'?˜"t
Öñ?ÙßjHÁbŽ?­Qs¤N~?æcÖ9³P?¨€ªÆþõ‡?¢.³›+?Œ' ¸,?Ðò}ƒ)|?§¢Ago Å4FGL J1811.0-2725¿âSŠIM/Àh"!'÷¿À9ëˆêá‹À;ZÆü©3k@Þ´\"~Í@vœ©ïR3?Ïx´‡0¶V?;:bÒ]@rpŽ@*;±±éG?ïّG=V¿¦©aD¿¦SÛÓ¥Ú¿ëˆÎ™«¿ÖЀáf⸿äoTˆ'UNASNone?ºZ¶âæÕ/?²!Z
#SÎ?"Ÿ1fÏk¬?'ÆêÊ9[?쯘l©ý?³¿D!µ6?Î䣰,Ñ?¿Áµ'¿>l?w	‹1|?—Î
`æšE?çÐúíÑ®V?¿xfõF½©?ÑI!L˜Tø?ª®aO»?µY(ÒÉó?"›­jª¼w?ä°J?Z³?ªÜÑÈcR?Ӏ-´±(?¯%4šõÍÑ? ûà5ðIì?"èÏ®ª™?å0+"Hg_?°€¦¹ÁÜ4FGL J1811.7-1442¿íêE2º?þ	üD}ÞÀ9ÖÄÍ$À:ÿöÅĚÏ@ŽEµì¶w@Ã%Nn"?ÐýGþœ?Ùp ¤eP@è%@+i:?öcˆm¢Dä?ꐦv î?Àá®Ú÷³¿ÚڞÜúlm¿ä½ì)‰fF¿ì?韖]пïôÞcβUNASNone?'i2°ß°A?‡ûkÀt?¥Wõ˜Â?¢ÇNƟd?î7ò?¥"À_Uì?»m±Õfá?Àš(r±¿ò?À'—,5"?"×çxΆ?èrúE¾?Çý(6{n$?À5
]uíÚ?š³;7éû?Ç?Ҝüíÿ?¦SŒ®¾Ã?æ"ÈÁcI	?ªô™hG? ‹ÏÊ}Ãr?ÍNóSí?´"Û?£Bým7aZ?ìdÁç÷bç?¨×‰¾ˆã4FGL J1811.9-2336?҅8eÄw`À¬|•|ÔgÀ9\Úx†ú[À:¡?´‰	@ð"댫u@e€éŸk?ӓI]ìð.?áK.g˜@Ê÷	·8ç@g|"¤b ¿ØÏ[†I¿Üw†´º‡P¿è7¾³.–¿ç©ÇÁJ¿ïÿûÎBÓ?ïCÿ3QfUNASNone?Ŏíç½/–?¹TT.,?Ë>³éy?Ãtð2[?ãÚ´ÿc¹¼?Ç?»£À?Áf´-ëT?¿ÚÁÌþ<½?¶y½ëø-?¸K¸™su?è×7;E?Âyöôm/?Å-ðz:?¤ás]t}5?ÈǺÌP?¦™2^0S¿?ä®JU.lì?¬òlŠ?£kömó–?YNílk«?³Mgw"
â?¡ˆçhÁ:?ì_"°¤ß
?¤à<(ç4FGL J1812.2-0856¿®³xp‡°@ãâ"À9iÀv}4ßÀ;…nij'@I†¶º'@{©f–7?Ñ3a×5†?éU—¬Y¾@Ót62Áô?üq˜ç%á?ïðdìé¢Æ¿ÕUÕõjzÈ¿é®Æ¼èS;¿ïÿ–Aö¿è»À½Iø¿îQ9]ïŸ`UNASNone?Æ
ÀóÃÐ1?ÀàÂûփÅ?ÀòÒ0Õá¤?»åÁ…g=Œ?æ@›6ٓ‹?Å/ã"9÷?°€%«ÂC¯?µŸ7(†?ߦ؉™±®?Ï]‹7í‡?Ü9u½e?ÌFN£?Í°«Ó^ÍÛ?«óþ¶å?ÎlÚ{%C?±b¬'77¨?àøž‡‰ƒ8?².n×?Ãã)Q??hÑ·î>Çj?ÞÐÇvNn?ºÏÍ®ï'?àPŽEL#°?º"[üä%4FGL J1812.4+4441¿ï­3ğùý@9TgÓMðÀ;N'™ð×nÀ<Ž˜÷³*d@yòŽÖr@ ؽ›×a?ÇbY&D¿š+WÅ®K?Ó4ý¾1@ÊæÞpä¿å#ãŸw),¿Ý$	_$RÆ¿èr¦äÌÉ¿ÑÀWs"\¿è™\þØ<¿ÔðáxÚUNASNone?îì ?ŽÁ5?—×ËO̗ ?q¬5¢¯œ?m0cTÒ?ž:Í¿-X?–âéÃê­?ï$¿ú?¯?"9>Çêñ¾?Y4GÆ	˜?c®*X"0q?™ÔׄWxw?'Eb¨+?횎[¸?–`ÍZ_¼6?€út»‰"¼?rö×Ԁ¸q?±@ŸËýå?"ƒÚ0j|?íå±Rå*.?"*~º‡±?t!~¿y?eG–Çj½Š?¯ Êp…0?'ëÏm™Ç4FGL J1812.8-3144?ìj¨>ðM'Àýœk1˜À:'È-*ÛvÀ<0æl±C@Ž!AÄ¢?þ_æðd'?Æz>ŠJc?à·l³‡i@þ•`Nõ1@')ó?ïÿæj,Ą¿ãšÀá?µ¿Äx@Ùd	ë¿ã,æ³'à¿í…·š5 Ì¿íؾópPUNASNone?µÆE‡øì?«vž•ƒ¡?ܕa-µA?Å˘"7Ú_?Ýù
pLð?Äåc£ÌY?¾0ªK†¯?ºµ¬µkÌ?×lOózÖ?Ë'…ë‡9?àƒÕðù@??Ë¢ Cìcj?À]½%Fnz?£Žû¸ãÝ??äŒÌ	nò?³_y·H?Ï@ª"ÕÃ?¬õŸ¨gØÌ?ÒóµTNs?¥Ø°‰©_+?Õ©	mùœ?±q'°Wí?×cA>ª"N?­‹':hÞÄ4FGL J1813.1-1611¿´¸÷òò#¿?ë@dïmâÀ9.ð®SeÀ:J£Üºî@øÓ4ð͈@i:Áœíâ?ͳðÈT˜?ÀVT_þ˜L?õ-ŽxÔ'4?Ø٘,‡"¿ë³Na	y?ï2a|ÚQ¿æÙþäw
~¿äHîៗµ¿ë¨a}ÉY{¿ï¹úݬCUNASNone?ªÝ·i1q?µcñUtæ}?š©k]1s?ªw\Ih?í|Ûâ΃]?¹RŽCN?±?¥'Œ×Á9?°¹f´m(?£%*Ï?Ä&Slí™J?éþe¦©99?Å qDS?À\θl?©? ù«s£\˜?¿Ýs« ?¢!æý俖?çíï/Œ?¨TÀq5"J?ŒÁ¸å?~Y?	²…?¶M4Ñ=2f?§b†*ó¡Ý?ìÆ*a¹yD?©kn¿B{4FGL J1813.2-1128?ì&E9£˜T@Ȑã²°À9.@q	W˜À:¡»á¸@‹Ò@MM@SÝͦ?ÆðtöL?Ò}PbÃï"@ÇÅ&^?éÒ°;¾ê?ïO+.?®¿á<W3Ã{ë¿æÉvÁ}cX¿æORîº]^¿ë€uf¿ï³Ñ¾¤UNASNone?¥çï™ñ¨ ?¨Å[$iÈ?­+–—‡?¼HX6ßÍ?éö6 ß?"?ÀKèÒ,ð?­FVnu?³\OÅa§_?ÒÕZwN?Ì%·}ÎÖï?äÃþ"þò?ËoÙ¨"µ>?À4v7ØÛ´?œ ÎqC'±?Æap`i­\?¥ŠsDä?æZ†Yï]»?©µêC8י?y¬¸kmB?eDEXæÙ?É9…_Më]?­W<°•®?é~E7VfN?­Üw8¦Îv4FGL J1813.5+2819?Ыˆ±ŒKö@41ÿ?àHÀ:Ý\úŽ§À<­½MÓÈj@Püi¤&?ûޑÖV¹J?ÌðÔ¾Þ¢?àM´ôhó	@jÝÄkÕ?ôÐÓÇè·d?îßÛgšC
¿ãç- I¡Š¿Á瘋§"¿Ü«´NPÅë¿êtÝAäüÄ¿æPazChUNASNone3FGL J1813.6+2820?Ý×oʺ׉?Ã!CP3ú?Ös2àâþ?ÄõF?mÄ?Çjº©
ò?¸ý°qAã?ÔMetųÓ?ÏZd}¤{b?àðÛ¥?Ñdo~á˜é?ÆårßeÉ?ÀËá^¥?Üe"xNA?·r[³ÜZL?Ù~ á";?¸%§_,?ÅÛÍ W`?¥b¤=(Që?ÔçdV¡M ?§²]†:l?ÕÛµ	Äg?±ÒßB(?Õ<æ›Tíú?«Ç䗁¦ò4FGL J1813.7-1152?æã"î^íÌ@IÅÓï×À8—¡Vý<×À:I">¿@0êp ÏX@3¾sm¶?ÆZ"Zî
9?ÆkúdŠ™!@D,Ý®œ`?ø9€=Òô¿ë@tdUë?ï^µÍ¬Æ¿åßÁ œ,Ç¿è½^®(¿æ˜~±¶ÆÑ¿ï÷ýO0ÀUNASNone3FGL J1813.6-1148?µË6¡'?ªÙW-‹8Ù?¸ìæ§<–B?¸myÖ|©?ê(ÿ"Hy?¾oï{?§[Á;Ö!?©öá9M¹<?ØJνBI‡?Ïawˆõ1?âd܏ëÚ?ÎX—WØ
¨?Àþ[5~«›?¢÷Ž'óÂk?ÁÞÇS'³M?¨=ÓTKNÆ?çH·]ÖhG?¬Ó0»_«ü?–ÜAöV‡?ôž¬F‰
?Äc]ÉB?«S2ԍƒÐ?ê0FªÌ]?«•ER¼h÷4FGL J1813.7-6846?ÙT5SkYbÀ5Üك"t—À:ÂÀ<G³"ÛÈ@ȪWVþê@çLû‹&?Á.,¹•?ÉvÙ%J½>@]o¿«|@æW¢Ô*å?ï'È#ð ¿à€Õú¿ßìÐÃ|l¿æÜN_‰}m¿ë&ojñæb¿ïÿö$´ë/UNASNone3FGL J1813.6-6845?ê=Ñ!E¬?·Sa¡›å®?¹,Öþú9?²»sxÇ?¶1ŸöØh?§[Œ×—é
?éÍýg–?¹ºî¢A½
?²£dkŽL?°…ä.ò?¾ì³¡5?±žÐF}'p?è=ØæÒnç?­-Na‹æu?¸ÂBûµç?¢I8«vÊ#?Ã;C8im?¢‹eE\Wÿ?å›Ti–Ë?£×lÚÆ$Õ?Â&Øß´Ä? E<a'"·?ÇkÕ{Øà¾? Ä¦°£Ÿ<4FGL J1814.2-1012?ç™÷_>÷.@ÑăR/xÀ9u]ù°Z¦À;§ž?È@†ò¯	˜Z@$Øý\·'?ÓãҢϣA?ïÎÿ!]ȳ@v9þ(k?ÿü¢¯»Å?í½Aߞ`©?·ÔÂ]³¿íw6,â·¿å³:Š?‰ƒ¿æ4á‰t¿ïÿèîkƒUNASNone?½†²áá÷Î?¸\ru_ԑ?׿A`Ž&K?ͱûΨ(?àoˆó|­á?ÍH$êºâ?µ±ëkG—¾?ÀÉlŒ­®ö?âã*D§…b?Ïß=¹òj?ÔÍ0›ßK?̵ò‰«º?͸]þŠ‰š?¨rY~&p/?Ë:æ"?=?²]?Z'\p?áÃ.ßMœ‰?²ÂÔ£S?¢,ʵC&J?"bØN æ&?äìçÿßÔ÷?Ä|»îFã?Óà–©—ñJ?Ãú¶È"D4FGL J1814.2-3000¿áÌ
õÒT¡ÀΡáf·ÅÀ:ØC1­÷õÀ<mCÖïe~@0ÒĚ?ü}s]Å­õ?Ô»´4çh?瘒üÕ©@;YÎy@TÀœ<â	?ïýî½ãOñ¿èø¥˜«]¿Ó/ÕÜ¿çpi§Šô¿çg'…€Þ¿ïÉƽ¿ÐUNASNone?Õ·
¯±j?ĹuÔûC^?¡
þŸyŸ?¬!t¹z|?䙕7o°?ÅQ¸) ¹?Ìú/þè?—÷GT¤Œ? ¯iç?§;r~j-!?çÁi	ÊÃü?Ã׌bé¯?ä«~»WU?«¾eŒY
O?º|œ7Ð÷?Ÿ"îïˆ?Ð
Ÿô•NX?§3WR?àK<Î\r?°öåk¢'?´¡æé{?? iÿçæô?ÚA@*èL?±ZŸ'À²y4FGL J1814.4+2429?ÓTW=²Í@22ç³ØàÀ:vÉ5h—™À<‰a=2@'ìðٜi@Yã¡$¨?Ø1#ùÚL?Ó´B|Ò8œ?ÿàç6Ÿ?óDCƒãNï?åÉl|«¿ã¤­><%Ë¿é²¾=èÃοåq؊p0ë¿é+·sŸ4
¿ïÿÈ!ÂGŽUNASNone?å#Ñ(øÃ?Ç[fpÈ??Ï*Šq1½?ÇOøÞp#?¸ŒbDT¿ç?²áYb¶Ñ¯?á¥(¶Ji?ÏQSËY™?Ñ%feÀ]B?ÍS=þ}u?Ç [U¡m?À'F¾"j?äX)Vçs1?¯y.)•Æ?ÀrŽa…}?¤võæê?Î-G­Á?§á«_ÞŠ?ڝ2ø›?°ßŽ²J¥?Ë5MÙöy?µÙѮý?ØT»àåø©?²ûè¸$4FGL J1814.6-3621¿¬U?ÎQP7À!ëÒRGËqÀ:±šW.ºþÀ<,3øUÔ@dn¾Ï‰?ýAŽXø?ÒKÝcß$?Þ¼Øc@§"©GŒ‡?þ<sÿP³?îö+jçÕg?ï†G½Xæv¿×(èÁõÙ6¿Ë1··¿êJë€ìúj¿ïõXÝç¯UNASNone?Ùº–rZG?áu¯òRã?±ÄBKÑ`?¨¯OŽ8 n?àê2~«X°?ÄZ—•á ?ڛò'8>Á?ÌâJš8?«ºÊß©Æi?±$~ò?àöZ	iD9?Ìא-Ï>Ã?ãó¤"h\?¯œ$ÿŸ?¹¹'×r ?œ¨-õÃ?Ñ؉hcR¡?ªþÞ^Ð??ãa9/ÒB‡?²ÊCø·C{?¼éçùis?ª›"3ó"?Ò¢-?´
pÔO}Ü4FGL J1814.6-2537?ïdˆ=HØÀ°LÎå«ÁÀ:qó·ó ôÀ;±rGE8ï@Ï0֌"#@x~…A?ÛÉ{"P?æãèb)•Ñ@ãÈ\$Ä@ÿ[g¯¼œ?ì'1ÆK©L¿Ê™ú<œ"t¿Õyëñ@¿çýB`wº¿ïÿþˆ0»Š?ïÿ£ÿywUNASNone?Ôm».ð§?Ñ*֙¦@ã?Ãì•ÂÍMP?žôF`?àÍüø´X?Ï÷^†g
?ÐlÏ02õ?Æ¡¢ъ?ª­@òø??°Ü4Ÿhµ?æÄX·±?Ç[*|Ç?ÒµêÝd³¨?®»NÌm]?Љ‹í­Zä?¯D"z?ÜÀ‰4íñs?¯ÕI&¿'?×[ ½?´]DUüØ|?²¶n'x¦?¥òJ/ "?áûQrnþ?¶[h¯@èQ4FGL J1814.7-3420?ïVöҍ^«À uæ6*^À:xv3cÀ;Ñ[§Æƒ@®Qäy;Ö@ëE®_ú<?ÑgC:è3[?ÞcK©Í@.ã,?öVwî¤
?ïã&@©?Ô1½|Í°ø¿áÜ4-n¿ç<¢³Ï¿í}Sþ.ïÑržƒ
fUNASNone?¨âß=érÁ?¤ü‡aI9?åu/|(Ê?ÆpJœ¾?Ñùq¹J€?IJ–zÐnø?£u!÷z$2?«ÍþFTx8?ãÈÁ´Zœ?Í *Tí!?ÕÿØX\®B?Ëîõ"ÅoË?¿÷w/'?Ÿ!¶©Ÿ–?àϯAwa?±ä³å¯´?ց€Ã±K?®ïÕ¬åtÞ?§ªÚè`?x¶B\Ó?é ø_z?µèjQãK?ǶÑÃ%?µ6ë'HÆ74FGL J1815.1+5917?î¸!Qg@;Ÿû¹IbÀ:áZˆâ'1À<D|	f@×lu:(@¿\¢˜F?Ðb\ªŒ0?æ­z¹Â@ê±ý=­à@áð˜XüÆ?ík9i®ƒ¿ÒîÍþ¾a¿è̀†£пêòI^ãL¿ð?ïÿ±%§YvUNASNone3FGL J1815.1+5919?åöÏ؋5?Ê%9ß6¦Â?ÎÌñ¿³«?ǟˆ¾SÓr?²¯£©Õ›?²'|ñç?Ýá"BËV?Ϋn'y?ÙVœÕÕ|³?ÏÎR.Yµ?Á‰+Ïoî?³'ðp ³?ÚXᘰND?²qÑɄyi?Ö(Ló"êÜ?±þà¹è[}?Îý¢ç•Á?®nÜÕÕ®É?ás Š~bÐ?¸±þrœ?Ôjg¯E?¸×Ê<:Ô?©ë7?¤–Bä'H4FGL J1815.3-1336¿àyòAìÆ?ùæŠÁXÀ:µc#»ÇÀ;­iiP%²@h½}¤p@/%¿­*?Ն¼RV9?ï‹'!­@ØÜ@Þ¡@Ѻü•½A¿äúœl²±¿îd%ÿn	É?ÆÔ¨Ž¿äJæ
²û¿ïÿ¾[ðÁŸ?àRâ¥üÿUNASNone?¤8ë9g¿?¡Á|ÍsB{?ºQ³óy1?·À2bÚäñ?ër:ìþ?º]|5ËÊ?ÁaGúr?ÃôõS …?Ï0ÐÂÅs?Ë÷Nrûš?ãÛyëM?Íö˜%•uY?Ì(†|>Ò?«•[‡M"?ÒÄxu?±U«Õۉ?ßãøI ë{?±Ã4ˆC|é?¿>ÂeŒ?§;7‹Ôì?Ðç–X–Ë?ºq-a¦ö^?ã¤\‡'
?»ÒL.8»4FGL J1815.8-1416¿ì¾YÂi?ó2±-4À8¯Ö»cýÀ:<òô~Â~@ûèɂ•q@#¼ª ?Â-«3õÐÒ?͍eä@ûdg?ìiZ"›õ¿Ôû¿¾òCª?ëÄQh¨`¿æ9œf¿æ"‰!Q^l¿ïeDþ6ҿ撝'uÞ©UNASNone?™©?Éüs?®kúwúó?Ì|½¦æsP?Åé4IÿoØ?膗þ;I?Ç	£‡g¹†?•2j¿%…?~\i¨u?Õ*O²®?ËÕBÚaÍ.?äÁ&ðöý?ËÕìµÒ?·ÊÔOÉ?—ßÔD»9?̞´¢£#?®À>òBw?åßöv?¯.5©?t)Üôx
?b÷–ÚvÑ7?́zŠ*©‹?¶mSƒd?èwM£­?¶¹"óàe4FGL J1816.1-3908¿äûèÎWˆÊÀ$ù³ÃçÀ:Q¤nß±¬À;ðbMÒñª@P‰áÿº@
vÙ{0ù?ÌÂ*7‰?ÐGýûCÝ?ýVÝA‰?ò¨"pÃ6¡?ïýê|
<š¿åÁ`>¯¿åáù£Åm¿é=b.$¿çû¾Aě{¿ïñÁ—ådUNASNone?Ûw‰"ÎXÉ?Éê)ž$?žQO`~W?²'ðBò6?áQ°»ã)?É>ðª
¯?Ø¢øƒEû&?Ξ
ï8žµ?®ûڋ?Ï?³ü7ŽÒÙ?áÆd´Np?Ï_è}õ"?ãaóœDÉ?±gAâ!x{?µ¨@'ºpl?šÇ—:M­…?ÓÒ£Ѫ?­ÏÄ~y_Ü?؛P±æêh?«"Gîv?ÀêÍ{lÕ?¤*2‡>?ÞïHË[_-?°è˜[:4FGL J1816.3-2903¿ïæó£•	×À"ͅYÀ:"Ü·%››À<opŸM8@*ÓÄ[d@DEª.<?Òäç`Kð?ïÿûÎBÓ@Èd©ÍÄ?þr¥;¹>¦?ï'v1µ"²¿ãýô·ø¿Ò™#"™Þ¿ïÿâ£Î¦Â?ï؊p0ꄿïÿüoQÇsUNASNone?æ'Ü(|ò?Èa5èäuµ?¾3'¯cŠ¯?¾cbíhö?ÈFû†\:ß?ÂO0O/¸õ?Ìß¹ý1˜?ț£pŽj?´ÿ†¨4êÄ?À	¸/Ь?æ( «­?Ê*\	æ'?Ó·K~Úg"?±
òœRÉ?Ûá‹>Þ?´ÛFéî?Ðg´šYœ?©€rzÉ2?ݑf´Žé?ÅjÁœ¾×?Ãõ²§M{'?Å]|€Ǐ?Øs¿øC³ƒ?ÄÕ?áÞ4FGL J1816.4-0057¿ïC‹j¬Ç@_¾vÈ´9À:.Hè§À;_WƐr©@ïxŒÙ—¶@ˆ¹º¡Q?Ìzº0gý?Àÿìý)·?ö©Ä¿¸T@WKÐ
!?ÜA œ,ÆÝ¿æރ¾ôÚ¿æ¢:Að:e¿ãøèI*}¿ïüŽ[wõÛ?›^L€PJUNASNone?ݙú^úzH?Âñ
Ûç?"ŠbÀh¬6?ŒYÃ	Tã?à–¯º}{?Ã)ná߅Ð?Ú¢Dߖg?ljÄ-·"ï?£b¼¡U?§¼g˜ú_4?á}×çdj·?ÇJ«Û?ÝZ¶D…?°9À³àP:?²b7¢£æ?"BÍO?Þ»Ó:ºs?®úoÓ/à?ØÃO"t'?±Ç<üë¾?šq1ù'B?ƒßÑqw­?âÊÏ÷ÞùÛ?±ô.óõÐ4FGL J1816.4-2727¿°ŸÁ
Y!Àªä>šÀ:EžG~CÓÀ;ÕbþÒÙV@týۅ¢@58[' N?Í$ɍþ?à†ü©3j'@µÇ`c?ü÷Ǫfp?ïœQքܿá÷ ¦éŽ¿ãƒ>
É¿ÜÔ»%_¿ï
•µŠé¿ïÿÍ'ý UNASNone3FGL J1816.2-2726?f"ŸeY2?'íå<?âwH÷U?Æۍz>E›?Ù;²h?ÆbÀk?´Ì'ÜæòÛ?³õ—YEÍ?Í»&5UµÓ?Çý×ÛkmÉ?å÷¦
´/?dzó…Ž?Äh[K=è?£;ùDoë?ßÆ΄©×~?´"½ïš›?ÖÕ·4u?°q5ÞOøÔ?«˜ºƒ1?dÁm´†?ÜÉ°ýåQÿ?¶Ç}Ä(S4?ßÃ7±´‹ ?µÚû‰ƒsD4FGL J1816.4-6405¿ë'A‰jÕêÀ4ŒfçÀ:V#ßÙÀ<FÒä>@$þØ;–@›¸€®?ÀÇÐy)·‰?Ö°Þ$
%'@÷jøœ^p@eÍ=`Ó?ïÞâ¾ÑŒz¿ÜTµ"0ѯ¿à€ÎۚƿåÖ½•!e¿ïüK_ÏÉV¿ï'nÂ6ïUNASNone3FGL J1816.0-6407?ÖÛØõ*¾d?ÃŽÄöu?݅´‹¡¬?ņóOÙƒ?Ç<äÿ¥?Þ?· +ëX?ã‡ÐÓY¬?Ç›ÙËùg?ÎsGpc¡å?Åí'Z¿x?Ãmx€N÷l?¶%{1|?ÏÉvWgþ2?²úæ5""Û?á]нs¿o?¶=Š×~‡?Ê¿F²É?¨±–?·¿Ž?Ýdõ'3?«Ž!
›T*?ÎUÌñZ	1?¬®ƒM§ùH?Óp$'Ðô4?§¥ßéGqd4FGL J1816.5-1208c?èœ"e@Š	¾Å£
À9>'lVjpÀ:¡¨žð@þÓ xñX@!Äüó0?ÌòÇÞ%²?ËáÌ8RVå?ú€yK!@»t_οïòbüO?îþýÁ·Dû¿çIðäÚ	Ì¿áÇr_Ãßé¿ì|vÕIs¿×8\OUNASNone ?´Ñ }XÝ?©m×nèww?É
@Øõ'?Â"ê{síz?ç	`¦ø?⁥RJ:?Äk¼ÚºE³?ÀÝ?ò
?Æ©ˆOšw>?Æa"i'ì?å:®µjÐÅ?ÉcÕÉ»?Ã7쓢`Õ? Å¡IÍE^?ÃF®´<)?¥Ë®íXÅN?æ`Y.]‡?©ï³
	"?ÁfÔŒw?¢-&[8—?³ªg
ZI? 3oµÉ¦?éCä¾'š?¨m$˜4FGL J1816.7+1749?Ë>ùåߘV@/M߆ã´À:GI¡À< SúSÕ@@ƒÊû;u@XTŠ›ÏÕ?ðHÔÛd?Ðv	ý.êN@OÈ‹ñ:@¬ß¡GŽ¿â-ŸàÛwŠ¿ÝAÛ¢R¥¿¿ãßKà(IJ¿ÕÎN­=%¿î«A—z©¿ïáØݧ:—UNASNone?Ö܀jŒú·?Â} ÓJmù?Ò[ê_Ä÷œ?Á0pìVZ?ÖǕ5®
®?ĵáΔ]?çF†D$?ľŽ^¤?À1ÓÀ±Å?¾¿˜Lµ?Ãq&>m#?¶·/´e
þ?â"N8B
q?²ž3>‡øØ?ÈätºmMP?¬!4BkS?ÌÎRdŠˆê?¨ìx":e?ä)beés?ªN_ÚĤn?»5ö6q&?¢ðŠUÙÞ?Ðß½o—ã–?¨:­F¿.4FGL J1816.8-2800¿ßéˆåcOÀq´xB1À:fVߋÀ<
çbzH›@ë\ђ.@ý'$ZR\?Ô¹A?:}?ï¬Zœ-Ȑ@ &5?þOL'S$¿Ç"(GÔ?î¼ZYê
¿çoÚ]ÙúÞ¿ïӃüº{?êÿ}úâ~¿ïÿ:Þ"_¦UNASNone?×iÝ0&}?Æ;Ø'í?ÌÜêþèèª?ÂóCZDû"?Ú'­m[e.?Ç"ÊýR|?Ïøc˄®?ÉQªì…,?´§®—åˆ?¾ËeÖêú?ålñ::׬?Êíù¢/"€?Úq}L•|?­n
ºåA?͐ô‡1_å?¬vfN'š?ÖÆpUº?«¦'¢)Ù?á`¡OQMF?ÅÝíwÇ¡?ïªüÉâZ?ÄfÄãXDÂ?ÓfçâøtJ?Â1ªW"b4FGL J1817.2-3035¿×‹xÉëF
Àœ…×EÀ9oßq?RÀ;¸ò–Šñ@Øä|û@؛7(‹?¶¢bk/å?¯Åäü"Ì?ö-$[)'@²¹c
–l¿ÞBkØ?ïÿɯæ¿æ-'?2D÷¿â§Òw0¹¿ä³!96¿á'‡N={UNASNone3FGL J1817.3-3033?èÆÛm½?·µâ-âî¢?¥Ý{TÄT?‹ÖªàهO?ÊÏ֜~rù?·FJ×EŸ?èÿœßäý®?ÃôÉûÝX÷?h3|\S¨=?yÏRPÝå?Ë ¾Žúº¦?ÃÓ[ç'?çè1«R?°W¥×bÛD? ­'í4…?‡Ù5'ÙP™?ÏÊ®ž¾"?­^Ãù?ë‰þå
Ç¢?š,Fh}½?¢"'°éŒ5?‡6èu?ºž¿4üÓ?•B¯J$H¡4FGL J1817.5-1034?åþúÅ¿£€@³	ý¯Ã¨À:ÇíiûFÀ;Ù€9vC@©Š(b@ñ]¥Í"ƒ?ÒáO¦0€Ñ?ç»ÿTßUf@‡0[žŽ?ö7–§¡Å?çèQBgك¿²ªËÁµ¿Ö§e47?1¿ìm² {¶¿ïÿþó…õ?︣µ|N/UNASNone?°Ö¹‡â@ª?­ä
…ÇŽÍ?Ã^Ó¡óØ;?¿ØèôÐ?é
sæ†ÁÜ?Â
®°Ív?½œ=ÁǏb?ÂK£P«¬?Õc˜‰k¶8?ÎÞýSŽþ?ᚬ2ø?Î3¸\\ÒÎ?ÄÈxç6?¢¼:d'?ËHÄ°>à?©ZèÊ씃?ãûüpÎ6z?®ä$
`?£÷Ûe…?ŠwmfrŽ?àûǏ…æ?¸ìÜìÌýF?ۉŽnøÇJ?·ìão"4FGL J1817.6-3251¿ÎÈd¤*¨[Àžm=ðüWÀ:Ò7yêÀ<€Èþ3:@hÆøL'e@ÛÈ:–ÔÃ?Ö¬]᲍?ïô×x!yÍ@'ƒ'à@_VlHS¿ïöë¹÷Ýó?ïÿÄ;-Óx¿Áí@	Û¿íO9ßÞè¿ïÖ´!…5ß¿ëœm‰pVªUNASNone?»·ÓëE›\?³Ý7©§ë?Ö&Jþº?ȎAԍM?áuÅÝK·?É©šªâq­?·0òîù?¾1ÍÈmYý?ào§¹c?ЁˆNÎ?Úý5$Îô?βB '?Ìk!ðdÛ?«%ÔûE²?à{Â{=Ž_?³Áu@X7×?ÐûExŒ°Ó?­ÌA
íÅ?·Åðùq? ŸJýçyD?éYSòà=?±aJB+±?¿—oooçž?ªéJ†ýq4FGL J1817.7-2517?íHTyóÀª0À'+çÀ:–kÅJøÀ;¾}ík¨Æ@‰+Îdý[@º"¦6?Ö<€"Þ?àþ!†ù"@
X¥ÛÇ;"@‹4ԝü€?ïç¥*ÇSç¿ãe•®×ï¿á˜aÁ;¿åzJIˆà¿ïÿÿ" 5•?ïúµK¦ÇUNASNone?׃àýu5?ÄlýÅJ»?¼úÅPk"w?¸ãÇ⎹?àŸesÔ×?Å1¼€€R?ÎÒèαà?Å5çzø¾*?¤tÄ9S?¬6¤ûš¾?ç=Ú^€ó?ÅKŸˆß]…?×úÐ:ai"?°1ú=?È)ŠÃrÁ?¨"½Ç ž?Ûð¦<Ý?®î­ ÁE%?ÑË
œmÉ?±*´!½?´]2!•µ?¢"Á*äÏ?䙇Ôm–e?²m·J:1ª4FGL J1817.9-3334?×bZ]n›À 'ҝÇ%ÄÀ:Ø"r8À<(ÐV©Z@RȲ5ò«@–¦ Z?¸m]ôþ?á¸W=Ôw@ 7 þ}I?þÀd*
ñ?ïþÎ!`¢Ø?ÀÄ,[Ø¿ÝÿFÃ*¿äu/dÊ¿ð?ïíßlÁÕUNASNone?'¨]<?"†
¯ÊØO?ín,×ïÙ?µGùRÏé?°$—éEÒ5?²wç!ܤ?£)Så¿F?©}Û7;{?æ8b$D?Éb²7lŠ?фd¾ÿ—#?È+Wóó-Ó?¯"Ÿ#Õÿ?–)øÌÑ?èXpí•{®?¬
Uß–¶?ƹ€´'~?§L£X°º?«©¢"P?"	¶¦?èëPRÄB‹?°ª2««?ÅhV2.Á?«×¹ªôÔÇ4FGL J1817.9-1135?ï÷g!4Å@+àXšËÉÀ9H¬A<
À:ºŒã¨±e@]ÆYÁ@ßú¦ú«?Õ4<Ëbj?à÷–oB­ú@
ŒWâ?$Ù@¦o¾(ð¿Ö#IüMmò¿Þz"@Ÿ¿äkŒ–|¿ê¹ÂÅâοèkœ0LÏ¿ïÿú¡œGtUNASNone?ÖA†qå°?ÞhÊs¤?ÐÅ98e?ö?ÅY™(°5?Øù@Uµö?ÇP@Wiw‡?´ç¿äKI?µîð_¡?ÅüA8€Æ?Äþ[[–U?çãç³(vŸ?Æç̪b°å?Å
û3Ò;ì?¡Ñ/WãÞ#?ÇêYIõã?ª2ì÷6ì?äÁݸóŒ?¯¦[FÏ?Ÿø±T‹•e?…@|ùÁ;?¸ô
yà?¦óʚÒò?ë᪔gT?§7C?Íõú4FGL J1818.0-1339c¿Ñ8ӎ»wÃ?ðWš5 Ë½À9?Ùx¬ºÀ:ZaՈ@­>'
@¸©õ1?ΟH/Cºj?ØZí!*È@‡#uP@î›×6ˆ'¿ïæ†|†c\?ïú^À՝¬¿à³%³A¿æ
ŽÏ;<¿í<ÜÊpÑú¿ïì¼Á¼ÎRUNASNone ?~€«r`V?zKtu?˜Ü5£ÈÜZ?™Yh0Ño?îüŠÔ\?IZ]t[Ô?°÷ì8	?¯Èé€Ì5
?¿™`
Z?¿ŒSÎʯ?éþWÚÒ?Âdä
p–õ?¶^€ÊPCY?'8®ž}c·?Åöš³²-'?¤¥ˆõ|¤?綉9Él0?§‰Ôóª'?¤k&'æz?•ç}*ƒ
?¤]H'Ó9Ç?–ëçådc?íy¤Äy­ü?¤©:O,?4FGL J1818.1-2000?ٟ`ôÈ¥‡À	 bvÞÀ9æk¤"ÈŸÀ;Æ¡Ú°»@)²~AúK?ÿ)¢üê³?ËæáK	Î?âÕm…>˜Â@)4AP,h@ŸJ(Åò?äT´W‹P¿è4%CâX¿Ês4j•Ë¿ÓìöÖBL¿í#¼Sƒ¿ïÿ·`)
UNASNone?ªln®~w%?¢­pyJ??ÚKQ÷ÿÈ?ÇpèŸyˆ^?á3ª?ÆÍûÈë?³B{ÃB?±<Q.2ªc?Ä&-å?ÂØÊcÓ?èŽ%_.Vú?ÃpVý¼ ¾?Ì°ˆ~ÿ?¬.©8Z*Ç?ÙI¶ðžÀü?´ê4=̘?Ø­pËXƒ?°:0¼hó"?ÈÅe%˜–?¢ÒAHgn¦?Ñ…¡C¤?´?8g:xˆ?áGcæ,ø?³¤˜š-9y4FGL J1818.3-1233?å+UÎ釙?÷Û¼Ú'.À9'0¤ãy·À:¶]këáe@ G9Oó@ݙÙZyÉ?ÊüÑâ¶C?´Æjˆ	#j?îXþý–ï?û´¦xz:¿ïç܈+³?ëÍ$ Ҕ?µÖR²÷¿æ­
$F0f¿âù!°:¿î³©æ÷UNASNone?®/¹p˜þ?¤kŠ¸t?"N¡ƒö¶?o™ý6??í|WøIEº?¬,vƒèÆÀ?Ù®þQ®º?À™b1RJ?Ÿtb½È3?®'Q§ãáÉ?ê!U¦?Â;هdÅ2?Æ×3z O˜?£Å:vW†?·P_c	øÉ?Ÿc]ƒC"?ç`'5­?¨>méÂa¾?ÀÒºÁÐ2?§¡Ï§'ø?š"˜®…I?t$ù³vÑ?êú<ŠÇS?ª]JBøÓw4FGL J1818.5-2036¿±â+ÂqAEÀl²
.À9ŠºÅ­À:Š@aïß!@
uΎBù@¢ÍbJ?ÑEäü"Ì?Ð0üw?ùúYÍÑ°?û輻@-?ÑE0¡2•)¿ç.yÖ¿èÿat¿ì<ø¾îì¿Û¦¾%6™¿ãi¸ËŽlUNASNone3FGL J1819.5-2045c?Æ3'½àÚy?¼N˜Ã]'·?›j¡ä~B?žv½(ái?é—Ƈ˜¥o?¿9F™Ý¾?Ñ,¤øØ?ż/ùˆ?–
÷7?Ÿ›»ì´üË?æ¶U›Gš?Å´bXùÑw?Ï<ͨŠa¾?«O]b??¾ç§éªZ?¡÷_¼ç8?äSט«RE?®•£l‡n?ÃÇñ¸"?°ÄÆA	.?—«0ì5A?ŠþùóN?êPªn¹?²'í!Â04FGL J1818.5+2533¿ìœ‹¹dÄ@2$Édb€(À:>"i®ðCÀ<ôËÛk@ƒ¸x¬äû@é/n'"š?ÈHLŠr4P?ҋÃbjÙ=@ޓ@ºs@Š]sùvú?äþÍûÌ¿à)F Mgè¿é±'IC?ñ¿ç-'àAõ¿ì`½¯ùWo¿ïþV²"<cUNASNone3FGL J1817.7+2530?å"Ûâ·J?À°ßµÓ?¿éÁ̽!?µ
ÔËA	?ɾǪ\K?ºêè
<"?ê>{«¼S?½&Í%ÙÂ\?±7"Ç´Dw?²†Õ˜baR?¼ÔÿßmØó?²ÞÆÊ¢B?æÕ®Enÿì?¯pµíZ?·ÃþlŠ 	?žôƒW£BŠ?ÈÇG³þðM?§_÷õC‹?çÝV
<?¡70k…Ç?´TÀeFÆÒ?'	{ú€Vz?ÉÒ*u(‹¦?žZþøG4FGL J1818.6+1316¿í@ü(sÖ@*fZUÖÀ:h«=0À<€à,@ÐøÇÒg?þ7Tð]?ƎNâ¼"[?átÝ!®¦q@mÝS,Î@¡ÀM|€?ØîBþ­Dœ¿Üô[艿ЏÊB®Ñ9¿á›þÝÁ¿ïó6>¿ïva0FšUNASNone3FGL J1818.5+1320?Ã`†Óhy#?¸kbíöá?éYa'
?¿/ùÃf¿E?°–Ž"ýo?ªiæ"Uß?È1ŒÛî	d?…sϓ8^?ä?Í@öïÝ?Éåý•Ê?ÆÏ> 67%?À¼£³?̸6?®yÉMt;?å(NY›pæ?±+嬧M¡?¾ýX`? ?…®¤yÁ?×Ú>.õj·?®£{œ·%?ÖÍä§S;?²?Çï²
?ÑWÝÎcB?ªKÙ"ܞ94FGL J1818.6-3206?çïO¦†gÀŒ†‹ŸÜÀ:#R©@À;Ûo¼P}Ç@—%'Ænd@˜{0›©?ËJ3•XÂ9?âîA'šÈ@å	9d¥œ?ÿiÅHŸ6?ïÌ¡-â'Z¿¬ñu?
e¿á±Îyu6ä¿è™¨èÁõÙ¿ïú×lbÿª?èøª O€ÇUNASNone?¯iC
Ó?¥žÎÛ°Nþ?ᐅi•'?ÉÂlZ-?Øò°"é;P?Çô<J 5¶?ÀáHeA?¿æ
8@¡?ÙÅÁ#Ԑ+?ÎÞå_ûP?Þ0wë‡=4?ÎA†8Ÿ?Â)U$Ï@È? û\œ×Æb?àn­«ˆ.?³ƒëÎJHZ?ÖTAO??¯'ýùpä?ºÃ`ݾ?›ÐyÒo6:?á›ï–5_w?´€`èáî?ÖHœ%½?±ýxylÕ4FGL J1818.8-2255¿ì
P#êüõÀ0U¸™9"À9×	—XvºÀ;>|2€…Ì@š¸ý·ü0@÷GMœk?аiϘ?Ò «†+(@wºÄŒŒk@¶¤¬È"?ïɯa!¾¿ê~Åý0¿à"7É
û¿ãÁ9ñ"U³¿ï÷Q۔欿ﴟ¿x{gUNASNone?ÅHØ	+*?¸s.xq?'ÃÎÕ1o?Œ…´óP"H?êà"U³ª?¸ðVO	«?ÍÛÆV?¿á²\f#?'A՟8Ò?˜ždQìñ?ç÷0Kµ,?¿ùvQt~L?Ïí¡ÉC\?©Ÿ¤º÷¿@?Á×Îõb?ždþ}փ?ã¡!š=1Ñ?¬F²FôE~?ÌO€Ïۈb?«É²IÎÜø?¥Âµuj1?"N†5È?çôt²z×?¯ÞKRIÌ4FGL J1818.8-0828¿îiýÌ#Ò@
\‰ô
(xÀ9e(ÃnÀ;=ˆ ËR@¹·_­@Sœº¶?ÇCŒ^?Çãv‡pÍ@7}_§/"@"؊ñ
?ïàƒ˜¦T"¿êF]ýŒ2S¿ãq
‰U~¸¿Ý:(e#ñ!¿î©"ÿ+Ý¿ïæítãìUNASNone?­1·B…Nš?¥xظÔûd?•V›r‡w?'·!'›(ú?í'/³$Û?©aÚ VBõ?ΊKª#ªJ?ÂÈ]ãÝbé?¸?í²ê%p?·\ÍìYá?åUo_п?ŬÙ@Æ?Ð}r$.?ªùTH?½yvãÚ¼?œÍó5¤?ä8v?¬UI#È?½…ùµÀp?¢OvՖ°t?®á›¢7ªƒ?˜E·p"–?êa'"ÍJ?©©·^+4FGL J1819.0-1203?îCÐÒjñf?ùé5¹qÀ9h™YùÕÀ:"Š.‹@ÖÿU¶ú@)ú}	@?ÒÐÏ:æ/õ?ŁÛw_‡û?öýŒ£ ?ûe¦MC?ïÐN+Ý¿éx¦¿òÉ·¿è ˜'[Ýv¿éþ_
¿âˊw½¦¿¿ïûï< UNASNone?Î+LÚY‰?¿5RÐ¥àü?'kþ‡È7‰?@4ò°#¸?çéÌÕ+ya?À!`XÝ~G?¹õNVPbh?·È*kS?¡_0óù|	?©=F¼¹A?ë«c%ö[ò?»|R¯BÍ?ʆb¦¡?¦úÓÖA÷z?µ—¿ð½öc?—´Iý}µ?æ«o€>»L?¨ì÷Úa?§[•úQ¦
?áŽWË?'/Hېg?ƒIe<b›Î?íøÌY~e"?"d
õuÂØ4FGL J1819.3-0935¿ÔLò¨ç"@>°YÏ/À9n*†¼GDÀ:Ç'*ç4W@áꛔÆv@‰1‡aˆ±?жšÙ4º?Òiëáºð@±îúôþD?÷L³è$l?ïÿ••_x¿±úfch¿êñ´âg¿é¿ü¿ç׏³•¿ïÿ!é^ÓËUNASNone?ËÝtAG?¿ùætq?—>…'ô1?›¬4"*1M?è~nÞ?À±k_‡Œ&?ÀãQfz³J?¼6Åd™Qc?ÆÊÔ¿Œr?ÃsÀ‰œ®L?æv£qp?Ɲ¾iˆ´B?Ê&ºŠ´%?¥'°î(›Ù?ÂÉb^ü?¦ŽƒGþû?äÄ
Îàø?®\‡è~V‡?¡ä_hq~^?‡u»°Í™
?¶?rÅ#ä?ýÌ´n…?ìË°Ôk›? õºƒÙe§4FGL J1819.4-1102?éÿ)M×#h?ÿ_ì»"À9¬m&SQÀ:žÄüô²Å@HÛìû@~@RiÄ¿¸?àôC3[w?ඥxÊìù@ûç¢;(Ë@£;Xñ‰¿ïðÞú̺X?ï7ÐQ¿Ø'k>gnÏ¿ê'ÂIÇI¿í}tՔòk¿é"[å$xUNASNone?µ˜Ûؼ?®lñŸÖÿ?áÊeý†Ab?Ì¢èŽ`@?×,Ž3?Ë
æAY?´‡&ãðË?¸èˆIíE?ÐÝ¢O?Ëg»'IÆ{?史²|>?ËÊ8@v©?¼L
¬í3†?–'£LUÐÑ?ÌB×Ñ??«*/#í˜Í?åt­"›e??­0PèaÏ?¥å.¤ò?ÜÍùGvr?¶
4,Ht?¯
ï8éá?ëí['ž£?°0|Œ	n
4FGL J1819.9-1300?ß9Š/™J¿?íØ⟜èÙÀ8Ä,5èðÀ:BÁE°
@ÎÍ&8ú@×6žË2?Óí¶Üöe¢?Ѽ)çZ?ÿÄô@¯¹?ùŒ˜êS¿ê÷–¤ò"0?ÝîÅû¢MG¿ëõÄÝëB¿ê¯:J~©S¿àvÎ}üÛ¿ê¬çŸaÑUNASNone?¬º•Oœ?­åX)ëW?˜‹M'#"?•ÕÖz.Ò?í½ý"¢x?±§2‰íCÓ?¨ÈhÐ÷ñ?ª¿òq]àÏ?ÁPÞH¦Ê?ÂáFô?ê2e;^dO?Ã0Qø"î^?½Û›ÆœŒ?žYäÁiå?ÁÔU÷І?¥ðIéz¶Í?çÏw®{­?ªõ]ëÆt?'ˆëzïdÑ?~'ÿµ98Ñ?§9'XÙœ?˜°x£™Ú?íø ~šòß?šŠ×ò¸[±4FGL J1819.9-2926¿ïÔ#FÖqÀñˉ֮À:ª3DÐêÀ;Óà{Ö:@˜p¤ý[@¦k|OÜ·?ÅÊE
K3?Õ[Á<ëÙ@g/3Ê1è@AyúíÇn?ìvµ~|‡»¿Ð—¿ú¬Y¿å7ÌÎû¿áFJÂpþE¿î^%"ôÆç¿ïÿÿ^ðP`UNASNone?à63€|Ï?Âãþ°¬S	?Â;pjˆƒ?³§ÿ¶=¶?Öuá¿ðÂ!?Á}	»Iö?ÔîúUÉå?ÆC%tß&?«³A|WÚ¸?¯zU¤7å?ãÍN½Uób?Æ¥7B9ê?áÿËoâ×Ù?²¥z=2†?Ä  ŽNî?§ÕÉ·ãÊê?Ñ°ÙA×?®4¦Ñ"a…?ßéÚgF˾?ª$'¶Ø"?¿¥6o3?¡
æÈ]²•?ØO$ïk˜u?¨hKìš4FGL J1819.9-1530¿ïȼjæ#¿ÐWÁ•aüÀ9gLÖÀ;#ƒ×u.@FÞá¢G@í>" 
Q?̾­º¸Î?ïÿîbHÊt@Ôb^™éK?õ'{è-Ñ?å³ý">5Æ?ÝdZÝò%?Ѭ{ÃŽ¿èx²>@ÿîR¡)°Ó¿é©ÃGèÌÞUNASNone3FGL J1820.3-1529c?p<H+ñ<ù?npÄŇ?â3Æ\M%?Ì!UÇUq?ÛW'& Á?Ì}£G?Yoãû"?",_²	µ?â4¬R"÷ï?ÑÁ´ð?ÛÛâFðF?Ðßtßw†q?«Åéò¼¯¶?Œ=ޘÜ*Œ?ÜöƯ².Ä?·Úü ª|?ߐ|ö;F?¶²›è'N«?6"£æB?0¨(+YÜ?퀒+˜"R?¨G€‹oˆO?³äÚÿUJ,?¨3‹`²4FGL J1820.3-2646?êå®ðîÀÀƒëaãIçÀ:-îÉp!À;uñÀ¢@Óaš#Ø!@¢¢dCvw?ÔLÄô;Q?㥾/ûñ@©Ô•*™?þ"¡Û1"x?ïý
<(¥;¿Öy7¤\U¿éâL@Jrë¿êÞ́®Á¿ïá¤_Æ95¿éäL —©UNASNone?Ôð¢FŒk7?Äo«lõ7?À2óʝÌä?¾Òœ&•½ç?ázñêW+?ÇãUí+?Åõu†­Áâ?×6´2øÓ?ʳò›V´û?È£æ¢CÍÜ?ãÕ¥÷~âI?ÊPwàR"y?Îg.î†?ª6'í֝?ľYþÃÔ??¤G9› °?ã6¦t"io?°`Œs–Û¦?±F±\#qB?ë8"-Ý ?ÜäZY?µQwËT?ߨ:ÄèÉV?´ÎraD4FGL J1820.7-3217?ç}saÀ wB™ØƒºÀ:"Ô+|À<WÔUWJ@$‹Å¦Ê?þÖË8x'?Ñð\žçaN?çmjW@KU}
Ú?ÿ§‡ Q»?î[õÊd?î±ã<zÛ¿ÆQ$ŠÎÑ¿àGóÿÁ–¹¿ìUŠÁ9›­¿â]ŸˆUNASNone3FGL J1820.4-3217?ªÅâ²®?¢jŠšc#?á1A¢cqb?È>Èܼ_õ?ÚDÛ¾øFå?ǶJ:ϓd?¸o~^ÿ?¶®WGÀÎÏ?ÞAÛ|g¥?Ì0½ìüs?Û¢Dëø['?Ì
"8±Òä?ʍ'¯ìuô?¯ô)Ê8PS?ádêÚE†^?·ÀßEœM?ÏÞÂæýp?­cÖJË?ÎHêŸÄýN?­p  ¾?áG—©r±U?¹¾s[ol?̘¶ºp=_?°¯5›ºm4FGL J1821.5-2531?ê-aÉ.ïÀ&,ýxÀ:úmïǤÀ;c\Äüô³@àû­àÎ@4@^"àÍ?Ìj(è¬|J?ÉÙ¢Ò1f@8ݗl@íÚ£úñx?îÿü¿¿Ó½°d·9¾¿ê$'ýuE¿ßL‰°îIõ¿ìòSš¿ïÿ7ûþéUNASNone?Ïz8Ge°?¼yˆMÌ*ï?´DO΁?¬"·ü͋,?å˜çü'ÿÅ?ÀÄ="€?Îÿ²qé°?Àkt6½x? Å»'Ðä?¦bi¯ð4%?ç>G͌F?Á+=eé8?Ô~‰7…?®Uá¤ÜC?¹³ðí‡
%?š…k^—ô?âŠs³'ù?®2Š°‰­?ÒWsËîq¸?©Œ'ٙZ¢?»ÝªÏhËB?£ˆ.å̀]?ãXÀ­»?®›â­Oœz4FGL J1821.6+6636¿å4°k¹#@;ª% Jù#À;(o`àëhÀ<Öö¾7ޔ@ è¬Û•½l?ühžŸ'×Þ?ÃÈÃRЇl?¯©¢?g¹?íýú1@	ĺËÃbk¿ìÂmÎ9´W¿ïÿúâô?ïÿíUÙPi¿åØQÀ'ô¿»OÐ^
¿¿à^¨A}"ëUNASNone3FGL J1821.9+6636?ëÚ,ÑÒúñ?Æ!ܧ;$?r¡ÆcÀrg?(y»Ây"?À>…–©?Åkϝ¢˜?ï"ùÀêB?"'¦ƒ_?FAŠL^Âf?^3%¹#0?]w –J?'I–',
=?ëðš/ªÂ)?¯‡O'G´?b¤{°æZ?Y	yÔy¼'?¿æ
¥"»Þ?¯‰ü§‹?ï›çW´ßF?wdp,"Û	?.ì(×.ã?1àzŽCHâ?ˆŠyrŒÑ¾?wA²tfª4FGL J1822.0-3146?Ì6¨™ÍØÀ ySyú—áÀ:•¨þ'j÷À;ã)þK@ႁOù@4Ÿå
5s?ÊoEFl?§¿^5{ž?⦓}æO@>—…BI§¿Ú
ý‹["?ïþô1•¤B¿è@C=¿Ý'œdÐK¿ëëÌ!+HÙ¿y¹!/‹ÅUNASNone?Ú§Š¬:\?Âå&DRµ?©ªŽo?¦"p©†^x?ášîHR
?Ã-_'1FØ?㎷¾—…'?É¿èÔn¼?i¨J\'?x¯'V®,?Ø°c1Ò`û?É®³Ëº?ã…íĝ,µ?°³üÞM%ª?©¼ßuà÷P?'´:à•¬?Õ¼ˆˆ	‡¬?®£"£í-?é·¤c˜"?¡¨ÜõLœÂ?•$žë8W?ƒGí€i÷?Æ|ڔ6®‰?¡F·f"x4FGL J1822.6-2502?ÙR•
mÒÀ½Û˜A«À:q7öçRŠÀ;…yB=K@ÞM¨ªY@´ì O*à?ÕÚ/¡XTÖ?à"Ìô9ù@Xæj,Å@°
©¶È¿â!֝l¿æð+¬V4À¿Üɀ2Wk¿æ®°:Ê¿ïÿϞcWé?äæ»@2uUNASNone?ÅC¹0ÕAí?·¯¡ÆÂè¹?ÏHã÷Í?ÁÂ<ó4îÑ?âíË!'±'?ÅeÙB"ú°?ÊލѪè-?ÄmÁwn?­2>Ý©%>?³èô¿³Ú?çu8º³¡?Ä·M«?ŸL?ÎTk÷^~9?©Òc>BOK?ÆAyËy€?¤——môI?âچJÑ?®¨Ë?ř3¨¨£ò?©¨ÛR,t?½=·?¬kH³r?æøKb2%?³òÅ¡A8î4FGL J1822.8-1118?æùóZ}ã?ñ&Y0þÀ8çíåÀ:TK8ãv\@±Õ>ì¥@ÃJ‡ãŽ°?Æ~Jž3Ý'?ÂƇÕvê?ý¹|X@2ö?ÿì0àr›ÿ?åxÿnw­¿äƒÛÂ3¿è%Ò݈ó¿å'úhçJ'¿íTvyÙಿïóܦ^£úUNASNone?šƒ¬U¼'?¨	ê£.'?ž{8G""á?£—}ñÙR?î;' a-u?°¸)-g+?²aâÀ"¡Ø?­
¼é"ˆ5?°íƒ*×ä?²1Ï7¹õ?ë–B"oC?¹Y]ií/??Å7½uÞ|?¦™+RŽˆ?¼p³1 ? ¾
Áp?ç$j'_?ª›'y×#?¦Jü²³€?Ä«Àˆû?­J¹›²…?"3\ÿ´ëœ?ìƤšû×?ž}V³'BÒ4FGL J1822.9-4718?¢†:5=ËÿÀ.,ê(þ&À:cÞº5"À<6%ðT'R@þ 8¯žê@!%‰Õ?Ãÿۂr5¨?Ñ'ýž%ð@	N½ÅÈ̍@¡ØàVls?ëJ%󯏥¿Ý(¸ÛÔ&³¿ÞÊZâN¿+¿äÁtæX¿ïÿòɶ—׿ÉÅèª;}UNASNone3FGL J1823.2-4722?ä倣"Gß?ÀuºpTw?À˜7¤jå?µ. ¡?ËÑÅÍGû~?¹ðëq›üÅ?ë֘Í^A"?µZ•vÓ±?¤Sñ%bυ?¤ñ6¥eÐ?·!A\‹?°¾ã­[‡?ã®î»+²y?±_Ç%°?•?ÅN€Ùˆ)#?¦ð$8DÐl?ËõÄ9Éü?¨!–"zä?æd4xßD›?¢HF×CÓ?´ŸÍ‹!?•T4A?ÌbÞ5½-? ™Ìí­Á^4FGL J1823.2+1209¿ïÆßëb@'eÿ'+¾ËÀ:Ó°QlÀ<ª¾
'*:@­B§šcC@œa½Š9ª?ҖÞ­?ïÿ¤%
ւ@D9ô"?ûfkâ|·¿ãÉ¢
cB¿âɹòÕu?Çñ½_œs¿éÒ¹
x)¿ïþdž;îÄ?¸xQJuoUNASNone?Ðrae­»?Ã2δã°?ä§c‡+?É':ô?¿R9?MÄ?¾Q*^þ?½>Bå=Û?Åe善¤ƒ?èU³ÆÁìý?ͪóç>RÛ?À
rYÊ ?À)$Vòí?ʖ©@ô—K?«õ·±Iª?âs»°°l?²˜?#ÑP1?˚güJï?¨äÒ¿'?šA9+€E!?ŒVQ§)Ñ?ìE·$‰ó?°}·Ú_Ã?¹=ƒûûŸ?­þ`­Šã4FGL J1823.3-1340?ÓþˆImºÌ¿½kW½VÀ7d_4Bý¬À9Ðè±.á•@VIã£Ô@0k_Êjó?¬b¡œ»­?ÏWŠý@Áæ??öÍþîˆx?êÔ½‡	Ÿ?Ó¸GD7<'¿à¤¸F-
û¿ã!½êÜ­¿ê
Ä
áj¿í¼ã`7"VUNASNone3FGL J1823.2-1339?g€'çŠâ?^'˜»P#F?Ùp}Ç-œ?Ì;›œ›ï?ã0@™'«?Ì0'¶¶$÷?uòž~b?%ѧT¨X?æÛìh+?Ä*à`†n?Ñõð+­6!?Ä 1H}"?ŸŒ‹®~¬?‰gŒç3­ò?ÛßMƑ¤?»ó¯?á
{¬38?ºZ
0Šš?FûèrMa?5šv¹æ7?×G	q'Ó?¹Q/¨î®?äV¼'*¯Ä?¹[îdeÀI4FGL J1823.8-3544?ïJGgPNÖÀ$³H+è¼À;!<ÝÖàLÀ<­‰;}…@³GC¸?ÿŒèæÞÆÊ?ÓÒ\Ä&5?å±	!ç±U@HŸž–Xœ@µy'=/?ëLѿкî?íVˆm!k‹¿Î-º"{*¿àò÷ÙÀÑ¿ïÿŒri©è?è»K€1ÈUNASNone?戻¹:_V?ÃpÞzÑÍ$?År´ã5EË?¾ðäWü»?Àj\7á<à?¸/\ãˬÍ?Þ"^[¶ˆf?ÎïoèŽ"ž?³ƬÜ?Âw<†¬t?؃âæ!,?Íu.Ï«Š)?àb(E?,h?¶HÝ
ç?ÒLG:'ƒ‡?µ^)zkÙ/?ÉÞÐuÞGM?¦¶Rïˆ?èS÷ø]²?°ŠUIŠ?Á‰jÎ,Ý?­k7S]ò?ºMl#v?¡J«ö6ÞU4FGL J1824.2+1231¿î;&L	ì@'Fd+ùƒÀ9ùžã…uöÀ;°öüK?™@²è @¬6|"ÏU?Å]b[¿ÄQ?Ȓ›ãö´þ?ýF©î@tÂâ¾%À¿ïÿ²'ž«Q?ïÿú Âî'¿é3¼$Þܚ¿çn¦`ýEæ¿ïõpŸÐ?s?î"úÎg׀UNASNone?íf;lADH?¯²'6È7?¥ mcïŒ5?¨/Z1"?¤{Û×ü/G?¡I´zì`?ê`šÔߏy?î¥ßœ‰?®Ò0è{?µ‰ÔÀM?½'%Ìëö?¼6Õa"•?â™í´F
?°ü,âÕ*?½Žö>q?£ÅÄS…?ӄAöUH?«É^ï+Ó?èNÈ.Ï9!?¯œÿê''?¯{¡ À±.?™Â•MÅD]?Æåöܒï3?¬íÍf@ý4FGL J1824.2-0621?â9­_ô@ÐD¡À›À9F¿'țæÀ;Òê šª;@ݕܠªZ?ú7#¸kì¸?¾‰/¿
l?ãaŸËŒÜ@!gÛ	¦qï@>Ašÿö¿îYÀGƒL?ïñs	â×Ñ?Ä+üŸã‹¿Ô×~×v¿èUæ¼b~¿ïÿÿ" 5•UNASNone3FGL J1824.3-0620?ªÙzþ}'x?¨ÁaOö?ì³l¿ó4=?¶»£í&ã
?©ï¹O"­?ªí?堌*?›Qå4¾"?²Ž©(vá?çw{­ÃP9?ÍGvkƒsµ?ÎÁçL'H?ÊÙ±Fù?˽`œßâU?¬þ6
~§]?âÀÝæÐuJ?³sÚ¾p?É?'ÇÞH?©‡/E©t?¢Âîˆá…?‹yGd?PP?çÖabmƒ?·WªÂ¹á?ËõÀ<>?µ"¦§q4FGL J1824.2-5427?à1qo·|À2Œ`Ëò²À:[ùæ
‹tÀ<‡²ù¼ïà@¤lŸ:˜W?ü~CÖ[?ŋ)ÿ­Ê©?Û9»n€'@Äq´xB1@ð¾'u³¶?îy;àÖÄó¿Î¬xCˆ–¿ Ó¢ s4w¿á™i=[U;¿ïêúêíID¿ïÿö$´ë/UNASNone3FGL J1824.2-5427?Ù^øÁYú7?Ŏ²qý¨Œ?áªqúrÑ^?ÆHŒ"¿sk?ªaN\?¤[x³P?Ø·€³'ó–?ËÍêè;[?ÝÇ.1÷à?ÌëB¯Ùa?ÃÄ<–)?·½ª‹«	?Á/3ۋúÉ?§/vWùï?æÎuHF‰‹?±&›0¾¡4?Ö÷Yß	?¤`|>:ú?à?€¬	1?° ´–Wº?ÑݸA¾{?³6¯ý¸?Ì'{.^F?¦tP"˜P4FGL J1824.7+2403¿ÌVñ9¤Í@0HÙºÀ:œÑ¦PaAÀ<\G4q÷"@Sûª°Ã?þh¤~Ïé¸?ÕH 'Áç?Ù¯}HÖ@‹ÔÝ<†™@a4-.6t¿ï§x_7H?åì¡~ji¿Ý¥a~õÿ¿ã'&"©x4¿ëȽhÖ®¿ïÿöÅĚÏUNASNone?ê8µFÔÔË?¸=ë¡?®äÒ=ö#?¤žHTê+?¾Ç칺^?´«§;Áò?êvÏ¥U"–?¼FÊiQ^?°sQÆ\_Å?²fÎE'zÔ?»Ö1÷š?±,iËÔ?åžÀ!`B3?°n.¸3¨"?¿ÙM±xÚ5?¡äxÌ?ɘX¡ÂŠ?¨ôà3,»á?çÙXXB"P?¥ÀogºÇi?¯, iˆóU?›¥'ýËC?Èϖ""±í?¢¤+Ñ)¢Ï4FGL J1825.9-3153¿¨îñãþ.ÔÀ"ÄÞÁÁ×À:"×`¤…†À;¾k#d‰@'ZïÅZ@ù4ºð!?Ïh`fþ?Ò@âô,@QáŽû°æ?ü†WÕÔÞ>?ïœÈùµ½¿åX=˜çÿãó"Çz¿æ:´ÒD2¿ïû]èHS?~+VUNASNone?×íf;\?¡YŒEs?³±ÿŸ}?¨j[©×N?âúfŒîb?û›?Ò
Ø®ˆg,?ÉÇ#xZÊ?¼ô> ?ÁÁè|о?ãZ‹æ¼8?Ë¿{SY$8?ÙD{	u<?°ŽdDYÂ?Âj²îMº¶? u¸tŽîÃ?݆+cæˆ?®GƒÞ¯¦?ΐØ;¡ô?©Ëâ´Öæ6?Æ,î7M"u?°á>‹?âó <¶f?³×®¸wp~4FGL J1825.9-5614?éùÕ	°À2ì|ÇÑ»IÀ:tý£.mÒÀ<W¿Úv@"¹._cé@\á>iÈ?Çòfh?Àkj1L(?ðu'a¼³z?þ±Naaï´?ïþ'¸«­˜¿äé5¹pß¿å¨tþ¯ž¿éžƒ¾ôÚ¿à2Ô¿ëÉú?KÅPUNASNone?í;ª²ŒÛ?¯H;,·î—?ryxµ¤?ž?kÈL'O‡&?´ûßU*?®£å"5Ü)?îN	"lKN?¥˜ØËîé?{+:´eH¹?"îíZ-h-?§¹ÿb®¢?£^֜?ëíHàF?¡~ýa£v?'P/¸L~?}lxBêf~?¼A³õ
j²?Ÿzºá?·ï?ë&ß?›ý¶1U¿@?—]ñp3ª?ƒ
 "À‰/?Áá6}'?šMÀš®|L4FGL J1826.2-2830¿qm¬wâüÀXpƒڑÀ:zyöf#KÀ;åµWeA£@á]'£]@\¢}méè?ѯä^¹É»?ávU⊤3@«4<Ëb?ó|¥³Û?ï";ÞþR¬¿Ð»ÙÊâ¿é¦î¡ˆÑJ¿âTÿ5Õ¥¿ïÿþ½à ¿?ïÿÞr¾"UNASNone?Õ¡Ža\?Åfæ-ì?ÑîCºÞƒ?ƸsGÜÔ?Øp."&Åe?Æ	‰²i–Ø?ǜO¸âœ¡?Çñµl?Π›¿â§J?ÌÕ £ñU/?âpÅ!ί?ÍmbVK˜?ÕÀcÖþâ?¬v ±KØ?Ñ3ÎB|œ?°ÁX<û<Õ?Ùο'ƒ?®ÊH‡(e?»Ø¹¸¤?¡W¨J
ˆv?ÜY¤Î'p?»:N⩪i?Üá%/!¾?¸°¦ã)øD4FGL J1826.5-1202c?ëN9
_0Š¿­Í¶<ù–ÁÀ7þ)›Ú¼zÀ9îõì@ß·Ú@¹Æ_ËA²?È
Áúá³?Û«;³´M@ϱÀo?ûFîK¢•Â?焓xhҿՔÌÀ¸ln¿æwóÂî¿ìNwÇ·º¿ïÿþÐñ?íì|*	üUNASNone4?˜ÙT.óÔû?³Àö6Ë<õ?zç8V±Âw?†'ݐãW?ïfíÚýÓ?´(³g]Í?¥
Zí	–?ªy~g±¬?ÊÌ©CÜ~ç?Ã4ó¬·‰?çü*­?Ôä``–$?º…'¡q?¡ó¸¥âç?ÿ<1ÄÍ?¥²ÃÆû!Ù?ç̀Seúž?­i
-\+?bǺHù†Y?WŸ›¹ª•L?½ÿâN?­W
úh3ö?ìM…º¼·?­Á¿ˆÕ¿4FGL J1827.2+4303¿Þô¥Œt¡@6RÿŸ‡ð$À;$;ž;¿ÊÀ< j0'|@áH—žl½@aÙ¿#–Þ?Ñ
#hú?ÇTÒª²E¸?ôu"‡!œ?û[Õ@Ž»o?ãìá•0Ô¿êi‡]æJ¿Ç9`¿Û/dý/Á¿ì=#vý_¿ïÿŽ@)çUNASNone?ìx3çÊ#?²Æúº€d?•²ƒÚÐT?[&Y鎗?¶ÑÀbŠúÙ?±[0f­¤S?íIb@†"?«"¥‰gL$?ÊY%-‹3?'‰HÅȔ?±¾ÉVŽ?¦òã
Jߊ?ì2^ò´'…? ¸úöÐ!?ó%4ÆÕ?‹ç…íÇ$?¶ðA!B'?šÃ'=#Y@?éúõ«ƒ3? 0e³N?£~¬€"Y0?ŒÕ~¿®Þ?Ã4~1Ïç?K.iåh4FGL J1827.5+1141¿ïß¹ÓJë@%ô‡ü¹$À9ȄÚ`3À;÷é"mé@@ö¥8^@+¢õÚ?¼±4u¶?ÖÒóW{@v!`¢Ø@Š¥ÜÈîF?ïøTÛ#§¥¿Ø*¬¼aË¿Ü¿+Žúg¿áÑýžPãr¿íê¬"¢º¿ïÿ¶>@£UNASNone3FGL J1827.7+1141?À	AkJF?¶ù¶Jf¸?贄΅¤ ?Á1rÖY?ºIÁüF?´;0‡S®\?Å°iÜ¡Ï?Á¬,@#?ã$æ%\ÝÙ?É8Ö& Æ?Í»þf¯æË?Ä`+1–Q?½$v‡'Gž?¦^Z>?û	?çN:‡%j'?°6~Ëå?Ä4ڟ¡²)?¤›¿ ÅÕ?Ѕ¼Ú+$j?¤ëÚªÍì?Ôÿ€Ph6?°füËRWÚ?ÚzÂÕlÆ_?¬ÄOÄÙ4FGL J1828.1-1312?î'(LWúñ¿íƒîÓTPÀ7酵·'À9s7+æ7Ø@"ž >¤V@mPes!?É!Þ!3ˆ?Ðå%ßÀX?þxøŠ.Ã?úaÂgÄ
¿ápÈà.(‡¿êé/~¿Ä¿åÝÐ?ÈíÅ¿é'9@=‡Ë¿íçÀn¹¿ïÿîbHÊtUNASNone?•q*1O'?§LRéé?s5F—øÇ×?…úÂ:'?ï.!E'ç?©­7xÊï?¤]²(\Õ?©"\rîË?ÂÝ
¨9SV?Ãä°ë¶x~?êâ3p]?Ä+ØJQTô?¼ýI«TvP?Ÿlñ™¸­?Ń]WíÒ?¥å…Rú6?æÿtš+?ªG*X†?k"ZÆ:Á?`§ª·¥®œ?£u&Û!Ëé?•-}¬2…?î­)Œó?•áD¤Œ'4FGL J1828.2-3252?ⓄM›ØþÀ#˶ˆ½©CÀ;)mã2iàÀ<¬ÝpÜ@ûàÖÄó:?ú®!ÛòÚ?ÕØá-,?å'Á)h¯@
`9[k`¡@Kº5›mY¿ïߕÇ}³?ïÿ;F',¿ÊŒbN~¾¿×<(¿íwi¢ò‰¿Óã~T™µHUNASNone?äÜJ?_­Ð?ÄTiìÖ}?´œ}¦4–?®LÁȳW?Ñ da×;?ÂïÒâj²8?æå0Áœ?Ì3ÎgÆù?ÀkvÛíÕ?§`¢3p !?Ò .çê?ʕ£D±ß…?æ†÷]ÔÑ?®Âƒ9é>4?¹×CG'? "¼#Øô‡?Èøšg)˜?§¹ÙbŠ\¹?ìCQ'6ïò?š½Q.Zf?¡~Ò¶^?`?$Uå?µ&
"øÅ?•­ Þ'Šx4FGL J1829.6-2545?Ô9rINÀ"`št‹À:unF.¸zÀ<HåC¼s@ÓÜäòÞ@OC427?Ó-&ÿž0W?ïþ
hø@!G'R?ìђ&ç( ?m¿Ýß<;±'¿ád¢A¿îqkGv·¿ïúYbqå ?ïå«@
11UNASNone?یΆ­-?Ð/®oãðJ?Å«yŠGU?Ã*eq±î?ٝi¼¯H?Í7x‡Ð€F?³çÛø*w?¿ð¸"¨Å?à'•ÿ}t
?Ò£¬N.?ÚÚ

N?б–\¬4é?ˆíˆ@au?¨Y…AÍãm?Ü8礪˜)?²%ã'Ay?Ö™•Z7?¯œ¿·wjx?Tžì??r'Y¢ÓU?ì܁h¤Š?ª8 ‰L?·*c••|î?¨ÐDlf˜ë4FGL J1829.6-4310?îíÅãÀ-Ǽ"ŽÀ;>@ÈG,À<Ñý¾Ý @zú*O	@Ôj»_¼ÿ?ÔãÌ"'áÇ?ëÊÝßCÈ@	œ?,eº?ÿSƒþ&áì?ë©È»ÆL¿ã‹¯Rhƒ¿Ä¼=Þ\í¿èwsÔãòƒ¿ïÿþÞ÷¿ìÌòÂ)ۜUNASNone?ëtöî¤Bü?¿Œ‹»ãj?±ÀA?µB¡øò?²˜›Eѐ?²3}¦P?áeCå[?Ñ(ìEKpt?Ñ t´«°Õ?Ω¼Ÿn!?Ç*
~mé?Â@S'œƒ?æ(ER?®ëÙÑX¹?Á#ÈP£Ï?¤
¿nÙµ–?Æ;#rçï(?¥9pŸ.v?ÔgBª÷t°?²lü(q¸¿?Þh[ÒþTÈ?¸^g½e™?Ê`Ãm?±—Xº'4FGL J1830.0-1515c¿ÔÁ,íÁ0"Àc÷¦•*ŸÀ:IVH1ŒÀ;Û¸øÚr@"k³bmˆo?ÿXß_vˆ?Ÿˆ¨}®-¿¸;øÿ…±°?ñ>Õ'å!@Þø4Y£à¿âž%"ôÆç?î{P}ñÈZ¿é|í'hr°¿àòG°˜¹ ¿ÔɎÿ·°±¿àz 9påUNASNone"?ЉÇ)A‰?ä©ëãs8?s\Ò[W|?qûŽô]Kz?ç"d[F¨?þ''ÖÑB?Ñ*ææÎ1á?Ê0øsá ?nÅÁí;u'?†ÄnŠØ˜ƒ?çKÆÊ««š?Ê÷"¬¿ä?݌™ždrã?³{[¡²ò4?ŸjoNB?…ðÿQF
?à>_¶]i¤?³{>]R?Ú֋5@8?¶Lg.Î?•¡½?'6Å*æ:?áèA¸Qû%?·5/Áá	ã4FGL J1830.1-0212c¿ï 
èÌ@
×õfI
À9?|–S"üÀ:́I@»²@Uñ3^|7@]gº#}?Êu¶e':Ø?áPVY¨èÂ@¥Õo2½Â?üLH=0?îˆ@
²
ª¿°†òÍèU¿¿äF­czù›¿é³©Xb˜¿íÙä"rÁ?ÐyM>!MØUNASNone3FGL J1829.9-0203c,?‹Þi$>D?€\Ê:8)+?Ô9ËJd?ƖhÌ!ÉE?åiuʈø?Ƭè¡[Íz?¯fÜÊXñ?±Šš%m?Û£²%ðÝ]?Îj"Êc°?à7¹ bA?Ì3¤5Æ?·õϹ6ä?"Û¯JscÔ?ÒqázF?±EîZOÜj?ãÈUA!Ü?±P~Içz?€aÕ¹
'Õ?fŠ¤/7ˆu?ÔÒ±	,U¿?±Ñþ¡Ã¢a?åU $… ?±Î‹MEÖ4FGL J1830.1-1440?Èe*`?Ÿ—ÀWµäRûPÀ:%ý®(`À;Y.Œ…¡@!a÷q'á@èû"°ý?®_+‰›Ÿ®¿¹%ya?ñK&õ7O"@)$衦?îçYޘ§¿â{ê'Ù±¸¿àÒZu—[Ò¿âðóˆ"xÑ¿åIׄ¶³†¿Ð?"$ghoUNASNone?ÈÙV®ÝhÃ?ºÊ#óí‰E?|°Z¸]?wê®$šh??éIž×ë¤?».⹦]¹?Èêÿ€Þ…Ò?¿Ó æÿq?xÜ.;»x\?†ÿ|¹«þ?铇ÃPç›?¿Ä•«Õé?ؤðµ-Á?±Ø+»±ý?¢Íð)É×?"­ÑY¡(?âŒk"̂?°«Ð~¾D<?Æé£VÕëY?ª,Ón2?—Ítý]äe?Ž,Ô@ûÇ?é‡+'_–?«ÊPr¸[4FGL J1830.3-1601¿ê{½¿ØaoÀ¥Ûüëx‰À;;?´JõÈÀ<«Ü'<®@&~Ç!' ÿ?ò(IDíoÛ?Ôπ0fû?ÂÏôŸy­k?æÒÎn|@Š'‰)ßÍ¿Ì[/ürù¿ïúÙ_­9µ?ïò×ùP¹V¿ë¤šéû±½?åg*¡iFÁ?ÎUå]gUNASNone?׸ûC-;?ÊÎ:~dr?[(ÝG7¸?_B~Ƕ?äbºÍ…?ÊÌãSƒ_þ?Á¿Ã؟[ô?Å°"/;µ?{ùºª²9?˜žU¤RgÒ?ëX"'Äó?Å­
co¬Ö?åªLC.Yó?«¨TD*Z?' N*¬ã‰?€žr^ô?Ӂb–ø}â?ªì·'îPÀ?ËY¹œŠ[æ?¿¨'	ŒÃ?H7×í»Ù?Y@oyò‡c?é#ƒ¢áú?¿ÁÔãîÔt4FGL J1830.7-1634¿ï«wœ¼LÀK~ƒ"×À8û6)‡¸ÇÀ;&‡¹E @P`@@̘å>³š?¸uË°4?ÍEɸÆ/¥@çtü+_)@Gx¶Ë¿Ä˜mŠ#!¿á*ÀH&¿ß'7<Ø"–¿ã‡ÄŸ×¡<¿é­Ìâh'¿ðUNASNone3FGL J1830.7-1630?ÏB·Í?À¤V·_@˜?¿:h;j¢Ó?²‡½Ö¸ Ö?äH28d¸^?Â1[ÒLñ;?Ãþê1Ëò?¾
£.ŸþÛ?°]•"Hk?²Û)sª-½?èô'Êaãö?À¯Ü@Þ¹Š?Öý9±Ý?°ÙŠ"»ªð?ďز6š?¦Vö@×3?ß·mó2×?¯°4`áí?Ëjî€%?¬ÔL`"9ƒ?³ïÚ7×f?›]chn0?æ§`"´»Í?³Ôàæý¬4FGL J1830.7-3219¿½ÁJü:À$K-
$F0À:M)¹6íÓÀ;ï>FŒ¬K@
ovZzJ@òǝ¸ã?̱¬µÖB?КtŒB@K/©:÷M@]i·?ìŽPrß?ïùâå=¿å>f˜¿åOÍ2MZ&¿ë)˜JA¿ï…õåÊËUNASNone?ݗ'5Þ(º?Ç
]â:Ïo?³5³@Ÿ÷?¬C˜H°.?ݤ¡]Q¯H?ǴܧR?çó‰þ¾?ÇÆhŸ{Í?"Wß*½ƒA?ÙÉMb*?ͨýö"Tœ?Æ/Õƪ?ç(Ú÷YZ?°¦Ž'op?®¯_ûJ?–Š—Ò14‰?˸¨J›ÖÜ?«?Ò^›p¶?è:–Ʀ>£?¦Lúâ=%Æ?²XyÄ/Dn?›LN¦<>?ÅéhOc??¡ór*ü³4FGL J1830.8-3132¿ç×#/"ýÖÀ#aE•6À:>üGä› À<f°b2úÿ@ø$ EŲ?ýÖjÛ@-?Ãöó<?áwT€	û@0tBÇû­?÷ŒÈ¨zÝí?íÇh¿‡¿Úÿ'}ž;?Ç؎÷Õ:¿â,Æœ/¿ëº5¤¿ïý¾1)UNASNone3FGL J1830.8-3136?—¡^}—ú?"·°½b«?éO¦8-á?ÀÝHzyG?ÇÍ;[¸Èâ?ÀààÒ]?¨ÿKÐëd¨?´‹Ø¾ë—¸?â*«[ÅÇ{?Ð|xu5h?؊¿ÎWv?Ï$•ZI1?±±&"?—q0p#@J?輩ßušj?«Á¾–3`?Äÿï'Ë?§I@f…?µûû1ѧ?˜ÉÒ«‹z"?ã*ï7«·?»`ù'Z(¿?Ô|«U>Ë?·Ç)ψùø4FGL J1831.1-6503¿ïíȉµå™À6YTdÜ"«À:NRå€!ùÀ<‹Å£ãŸw@$Á'|D?ýŒMryš?Àúpßf,…?ÛRº·÷R²@RîcŠ	?üܼŸ‰?~@ÈG,¿•sG R›X¿Óðe£ráI¿ã˜a‹5S¿íçJýTT¿ïþ®û*®UNASNone3FGL J1831.6-6503?°J{#©n¥?¨JSñê?ìÊê
©q¸?±Ã¸°Íæ"?¢¼i:? ¡ˆSkÎø?ÂÜ/H
?¾^'½‹·?ç%@óÔF?Ä[ \²;?ÀËõfä?¶Y¦Áˆ%?¬ŽÉI…š?—êK¶
®*?ê¡ú)Ê8?¦gÁÛáŒ?¼©"rëq? gj>èµ)?ÇËÑúQ<y?¥n9Ҋ_®?á?­‡Z¢–?´—)õìß?њ»ô"˜?®ŒOoC´~4FGL J1831.2+0202?à3eì*ê@¬óý">6À9ž;1.v5À;¡]³9@sŸ4
N@7ÜËè¡?Ê]u&Ê;?º;²!""?ïwLg·Ÿ@Ñ#rJö¿ÁŒˆy‹²%¿Ù'k\ÅRÛ¿ëÝQŸ"ë¿âKu°†E¿ä0#̎¿ì$P±*UNASNone?ËÚ'+"eQ?½°˜Þ§ÅÈ?"õtF7€ð?Y &Ѥ?èaʒéj¦?¿8¼¹""?ãt8—ÒW?È|Lá0õ–?Ü`|cSg?–În…óq¼?ØÒ4Ší@¶?dzªÇSzÎ?×
¸ã>`?¯:ŒAS?³Á­ÊÅڌ?–¾'}2D?âíÕ%~?¯®(¤Xuï?䈔ûƒy?¶DÀ±«
Þ?Š¾"7V/?s4ãÞÖõŽ?ÖáèS7?¶qÆnîwO4FGL J1831.6-0223c¿îÛyaÚW@
orÖٖÀ8® HtäÀ:b4"F{å@~og–è@ñm*¥Åø?ÆèÐ#ˆã?ϏŠâq¤³@?òÿf}
?ù~‹=á7?ïh
?®–¬?ã"Ág	¿ã^PþJHN¿ævéki¦¿ê±ôÆ/¿ï÷™^á6çUNASNone3FGL J1831.7-0230 ?Ÿüv=?Hâ?šLkɪ¼?Êá¤"6¥ì?ÄÎx[žG_?èG³Eˆ\=?Æ&\(؞y?¤÷Í
g?§‡¨ß-?Û@웺??Íÿ³¨¢b]?áZAÌ?̥ˋ-ª?¼¬È´Hh?žÍ·o¼ú?Ç#ò³'3?§O²wÅø5?æ¡j<˜Óe?ª¬–	üŪ?€—³4–"?i\6÷P?È5 )M?¨ªc[Ä?é¹Ö¦«#T?¨Å1·{_–4FGL J1832.4-0152c¿åý*Hð@
û–C£Ã¿À9*螺jÊÀ:ŸFŸ@èˆòWuÞ@ŽY½
·ê?Å};‡õ'?´Œ5'î²P?ñ³WN›o?í¹ž"!­?ïŸÈ‡Ã®@¿ã³Ú°¿åÓZ'És¿êYÙUm¿ØCÑ(l0¿îûž ç×UNASNone<?»<x)?¼4ú،"?‹1í{§×?RÍ2œ"?ì3g©:/<?¼ýÕ>êJª?Âi¡m¦?¿ÿÚ9²³}?·³rŽ#¶ƒ?¿2܇»`¢?èo)Jw-Ç?ÃÁ!º(]n?ɛìRHã?¨—{'˜4?µ'lïòw?˜°co¤´3?æè·Mo"é?«V"*Ëå?—Lb)bc?"'w^ۛœ?Ú®æ'§?Ž¯¶¿ҁ?î\ö=»ª?" ÉN.Xë4FGL J1834.2-0827c¿»ß׿²\›ao܇À88+"Ù@yÀ9­¢uá-­@'£Ýë-@D@yJ?È%µœ.ŸP?ãÖ³ «Ü'@[WG9?ô'qº,Œ%¿¸ºË,Ž©?áÌ•¶¿áP‡×Ð6¿í7åžTê¿èœåžªÐy¿ïõ'àhUNASNone0?X(L­ö·›?`ìC¸¾Q?¨Q(—->§?¶ß`H»­Ø?înÙP60º?·*}6—M?ˆóNÇóÂt?³Rñ»~Ì?ҋú¡aþ?Çù3`0ɝ?æV5t/1ö?Çw›m±…"?¥"ÅñD?,½âZ?ÃXÔâs_?§?˜à(á?éÐ~hh¢(?©ƒ™—×j?:»o'Ø:Y?,¢À>CVÐ?ÑÄSUeŠ°?¸]šîß=?ç~ç\ß ?¸a¬oðl4FGL J1834.3+0613?ÚöÄË"@‰¼Ö_À:/ÞM'ÐÿÀ;èPÕ©³@,Eü
­@lKÅÑ0	?Ç·v¤L%?Ûê-/ãó@
Ew{a .?ù™²
ԚL¿äIq-iŖ¿ã»àÑn¿ßù;.ª¿â=@26ý¿ïúá¸\?Ôùr²¥ZUNASNone?¶HO+?©C£äÇãŸ?ÔiËV†BZ?Ã@rB\å?ã
ñAÔí?ÃvT(?³	?À!aešn?¾Ò	½?×(
cÐzd?ËìîâÔñ?àc·5¾\3?ʓî‡ayf?эSÀÒ´?¨Š]A&?Ó¨ëŽ]nœ?°2¢WVË?ÚÊᾯ?¯ÚŸ tÛ©?Çͅž|B?¥ëUóÐ"?Ô̪}T:?´ÿÝ1ŠMµ?ßL"t3m¤?²ùW3@ë%4FGL J1834.7-0724c?脈 x?Óñ(̧ãßÀ8Ní·þßoÀ9ógÁLf@CÏ*J+r@7õbLM?Æ('Á—å?Ýdéc±UM@_Ɨ(¦@I¯¡mÎ?ÖÔÀdïn¿Üœž^€>¿áWàÌV¿êÁ+Xô¿éûÔÂd"þ¿ïÿß~€8 UNASNone0?sÆ·ØC?q}ÄUGn?·~ú*šˆ?¶X}(Ú)?ìé³Jüu?¶¨ûÑiÂì?ŽEŒH™á?'€ô¤´ç ?ÅÀÞS–Vw?»>
Ó0uØ?ê³ìéGû?»]È·c7?§‡ö'–?‰·¾Ðøú]?Ȭ9Ÿ3Ƹ?¬%§¸§w?èdé&Ó¦(?­$?š52?dܸ+ªÇ­?RN-eÕl?ÂöÈF
™?¤²f‹Æ?ë-¡ÂÑÒ?¤Ðš¶H™Ä4FGL J1834.9-0800?×{‡MšED¿‹ò7jzr7À8²ò03¤À9§†P¹Œ@diÁºŸú@ÿ³Ä¾
'?ÃʀÂ2??Ú)åè
@XÁTɅð?úS—™åô?ïtôhó¡¿Üá‡ÚTtÌ¿å÷aËÌó¿é¤cOοïýv:ÂÊ¿ïñ`[_wUNASNone?—y+ÐÀà¸?³‰/ÿ?¬Ð({­Á?¯èՙ].?íw4¿(ž?¹>2nœ+	?‰¨L®¦'?ƒ¯¤öúZ?ÒÎÊ3J?ÄÀIs¹ºm?æ2[Üè+Ã?Äzj¹NR?ª¦gÉl_š?'õ»`Ë?Ð@ûËk^õ?³í±Dlc?æ5³Š‹?´ã`'õ?@é›P—N?2M-~¾Æ?Ê-·âú?¯ˆdTÒã?épWÖ3‰?¯"[[ÍhÐ4FGL J1834.9-2819?눣‡ÙþÀ"m‹`ñ²_À9ß)ã(XåÀ;¡?
×ÊW@A­RÞõ@õ†"X?ƃX$.]‹?Ì¿$³h£@©/¤2yÐ@jTXœÏ.?ï([žŒG¡¿äV¢¤W¿èû$Ų&¿ä¦^ê–¿ïþ×@Än?âÇÍSÛIgUNASNone?äEÛk?Ärf"ÕÖ?¤'íâ6˜Y?¢*DÿóUP?ÕHϸVð?ÃÍb;é?áÒÀ­T?ÌøI݇;_?¨;÷´ß•£?°¯‰˜«Ø?ÚÀۈ	Ò¦?̍œ'Ã']?ä1ú¥?²5ه`*1?°0	ܳ¹?"ü›DùI?Ӑ
ì>ºÓ?¯×ï³²ZÚ?å0çºYêF?«ÐË©ß<?¯)›s€G?•7hi1¥W?ѸýÜ(í?©%@ϲ²4FGL J1835.1-0517?Õ}5‹ä5…?óÄÀ:9tãë¸À;àæ½2%@¡ŸËŒÜ@N$PAa?ÔØèd?ïö?!}ÿ	@я1a@[î\>šE¿îäÍ_ê2?ï}ì?õ(?ØCôáé¿w¿éÍî \+z¿ìTÙÁQïa¿ï‹6môOUNASNone?'Çú=q?‹‰² V¯f?ÉÅKÞü;a?Á¶`ŸZ?èýÆÈoŸ?ÁùFµ?¤7ÉÅJM?«ÅcVžo¨?۴»Îhq?Ð0OËDx?àâ"w#?ÐI)øö?ËnÂb–Æ?¤:F¥¼S?Ô}¦m‹L?°Õ5øÚ?Ýõ"a)S?°æ©´žÅ?³rjÃuj? %X³ºáL?å%ÕÃ×
o?»•^œmê'?Ð×ÒÝ¡Ç?¸":¦½4FGL J1835.3-2439¿îaR;ÚÜÀµK 'ßÀ9¿WeA£8À;]Û8 Z~@2۞ ç×@‹@š?Ä2·¸=Ÿ?®h²ñÚMi?êHQY•?ýŽücé4?ïñ"aÔ±H¿çMž§öT¿ër4€:M¿àõÓ÷cyL¿êm)™V}»¿ÛVÂd>UNASNone?Ë|,`Å+?¾;Làªâˆ?‰]s"²ü?ƒµíë´¯Î?è¼»rª*?¿å•æ¿?ÔÄL‡ŽÈÊ?ÅA œ¥Ï?NJŸûS?›9]֖—Ë?ågg8Ã?ŝKòØ5ë?ÚǼÔä!?°|ƜO!@?­8T:av±?Ž•ÞDr¨?àȜ²ov"?°mŒøJ»?Ùå±o ­?°máÛt´?­‡â"ÀiÈ?'ëT8´D?á4© #¢ã?±*¹ð˜¸4FGL J1836.8-2354¿ëè×'™¢À"?ãDÞVÀ:BžHUÀ;¯ô"q<@
BTä2ð@ä¼B;
ó?Çè-%}$?Þç	úTÅT@*ܾ²W×@ôòÌæ£
?î)Xb—¥¿Ù¤›À»F"¿à]/…ÿ‰¿éÅ>=}d¿ïúȈšmÕ¿ïü™^
wRUNASNone3FGL J1837.3-2403?¼'
]2¢I?¯Bç¨X?͉®
M?Á!.<¶…?å,\HÖXW?Â÷ï:þ?Ƅ€^`ð?Ã5>²à!?ÌÐׁÐ?ÇHý^;_6?ã^Cê‡P?Ë`Ê#:'¨?Æ/¿:"?§s0íf?ׄb5??´ňñÆ?Ýd1¾@#q?±XÒÖ~U?Á‰
Ž€ý?šŠLI¶!?Ò ¡cïd8?¬ì¢=¯Û`?âMl
ä­¥?¬¹ØËó4FGL J1836.9+4439¿Ûå Ë3'õ@5!S‰Ò|À;
»DåÀ<Ì&Tþ_@ ìw‹§¾u?ý7†ª×¯?ÒQ/|}?Í|õžþ'?ö5…£BÈ@AÊ¢ûíø?ïÿn?x»Ô¿ïÿ"~LŒ ?ïó˧nn¿âº‰ yÞ¿ß:i]f¸q¿ÖÏo~èé8UNASNone?ï'm(ß'?—üHÙï…|?_v´BÊ¡%?]BM÷ëÄ?œxG·q?—âå'OÕ?î=DõÁðÿ?©«`7="
?w,ØÉ)¾?†ôái¨}?©FŠ¾ªÛ?§€Èõ¶ç?ìÒRG3û¢?š•Îhdµl?Š'I×<`?–A>Šø?¶$¢å;]?—¿>žGZ?ì©Â›P¾?¢œ`èöl?téR'˜å?rxÑ轐õ?¹cUþÃëº?¢JÌ7øG&4FGL J1837.9-0620?ê,L>œóÁ?¸Þm^'RªÀ8œá8"œÀ9ÔQžXE@äq–ñº@…à1?Ím6d@y?Ò¹–å	Y›@Ùs¤<ŠË@#ûó+g¿éMóÉøÝ?Ùä¼Îa¿åvÿ:Þ"`¿Ö=9T¿ëÍ/(·Ä¿ä?©þk«UNASNone?†v4{m¬ ?"ÊínÜ?Á5ÅÊaF?À"B®hap?ëXá<Ÿ°þ?Á*D§…?ðÛl¡d?¡º×û՘x?Ê3U=Û+;?Éc©†xW*?胣Õ$,¦?É ©š^Öó?·"8¿î±?˜OՄ²XÏ?ÍÙǟ×Ì£?¯^rû|¡?å—6¶?¯J*y¢q§?†;$8b¾¦?x#§øñ?ª0´#²ŸË?œ€­Ï£Ã?î,ãK	?žøkMrP=4FGL J1838.1-3352?ão4òbÀ(f¨ü
,8À:·?Úáb†À<˜úà@*¬C•V@茊½^?ÔzD¿¢˜?×c0œ*¬@|íáðJ€@u+ùX?ïÿÏ"èbU¿êƒÙ©T!À¿ÛÆ\Õn¿æÈl뻥]¿çžôí}F}¿ïü¥'†·UNASNone?íªs²ÍP/?ªÑ7:0ˆ?…ÀŒ9ÒpŽ?…·Ê¢n`?¯è¡Ä¶`î?¨wfµ	Ô?橁ºf`?Ê6é:
‰?'÷^Š@Ó?œ>æ§!H?Ñ}ˆB3?ɹ•ì[¼?èN·ÄÍ÷É?ª0ôŠeS?°ËߎÌè?—þâÇ!õ=?Æ_`ýºh?¤]âpór>?æëUԕo?¤à)íÈËF?›céÛ@O?…‰< ª?ÒG궢Ð/?¤ª" —Œ4FGL J1838.2+3223?'¿d¨wã#@0´£ø˜,²À::Å%8ž­À<Ñ%÷áN@°ZŒ¾iÞ@^P?³t6?Åòw×'É?Ðÿ ß‰@ºVwÜ?üºËÃbk¿áòýž%ðU¿Ñ	£ðÝM¿â͇<ŸÃ¿ê7‡UÊ6ð¿é5:ßÏÞпïÿöùŠpUNASNone?ã«È	'?Á˜ý5é\5?À>õ+`?¶}ö²g?Њc4¿­T?¿´pH˸H?äFÅÒ̖?Å~āch¢?ȇ
y!Û?Âúá0qß?Æ`'o'ò ?¸PÏN"_?䁲DZ?±Ë½èt°?ÀÅ)¨` ?¥€;(%ÿA?ÏÐ Gry?¨áqº'Ó?Ý[·Y÷X?¨(E=A¨?Èg‹ ûs?¨EÎa3ì?Öpƒ,(†î?«…•†û:4FGL J1838.4-0630c?ëΐ=Ç®!¿¶5U"…XÀ8ÖòJ¶ÝÀ9ßL¤@!7væfPí@ÙÒmrÊ?âh°ºG?¶'à~ÀÃ?òÈ4L7æ÷@—IEbø?æí½¨l›4¿ë,$ˆþA¿â*Œ 	_пéÇô@.C_¿êf££׿©½ï¦ìhUNASNone8?ŒŽÅÖWfÙ?'—gôÃO´?¡*	@%÷é?³!ødèêÁ?î{$T¤Bå?´ÕUK¬ú¡?¥¹J_|þ'?¯-­ÁÖ?˜M.z?¦u(ö$?íâéD`?³5Ä:e˜?¸è™ŒðÁÌ?œÀüL—;C?¸´xÔqæ~?¡òüz¦‡µ?éÌ]³Óª÷?¦–®²Ž%<?‡&gј?vâ?S¿?gÝ}[])?nÈM±ÌT'?A\w?|¥&´e¡}4FGL J1838.4-0545?פ¦YÞ]?Ïþçüþî³À8Pª<À9LWšÈÙ@#ì°	‡@1ó:ß¿?͖9'ÈÅ?Ù²…"êÔ@<¬Ñ"Âr?ôªm9>e?ƦÊYªì'¿ÓÁ*¡OÆ¿ä€þ "o¿ç¸ˆb½Þ¿îxIRYi(¿ïä$7í'UNASNone?WÍÁÛiÔ?Zï_"xÔ4?™[¿Ýý–Z?£çÞëÇY?ï); "^b?¤H‹3"'?ŠyyNàµ?' ÿ
6‡^?ÅSª­;­¢?ÁC'u%´?êA/ou'Ä?ÀÊàì9†
?ªL¬!¦Ûþ?ˆÃ§ÝðÏ9?Ë6*²Õ«f?¬Ìýj»‡v?獪'0'f?­ZQ–î?74räç?.¥ÜñÕ?±³ë1'? KZrqxW?íƜkŠB? Z'÷U4FGL J1838.5+3837¿ÂÔ
­V~¬@2áô™=SÀ:µÌ÷"÷sÀ<[]À¥w@"?6¡§°@Æñ'9y?ņ¢Ücm¹?ƒd·î!
õ?¼öxýí@õýÁ¿Îeô{'r‰¿ë]BÑ5è¿ãù½@gÏ¿â?õž}.)¿ïý'ÞZ"¿ê;Ì^èãUNASNone3FGL J1838.1+3827?ï-¦¸Ø¬?'Q܊ʶ?€à>ëþ?~¦øÃÜCä?'Û	وkh?Œ:ô°Ç$?ï8P€SP±?"vz»dI
?`²P}cI?pmMìÂ?–ß®+†=x?'Þ1
8ƒÅ?íCb5v»/?•×uµõ6\?'Åý[áï?'öÝw¤9±?±snýQäR?'±TŽxA?îÇïÄÿ,?ƒÕD19¶?}XX]ä¿?i&´ZӕÏ?Ÿ«ñH¦¸U?–É>踆4FGL J1838.7-0601?áL8±–?°uÙöÖáyÀ8öþ	…»À9ýtšÜ¸@"Ž3ºí|E@ir¥9

?ÏufI
5
?µú¥D"?ðŠ"˜±<N@֛öEŒ¿Ý(âø2V¿ÀQ°â5"·?ͳb(¤9¿ß¼¤`œøÊ¿æ{ï?z¿á©ø!mUNASNone?wNëPÌ?qN‡ý®}?YÛʕ²e?ff.¥g:?ïÄtDŽÒ?wgôÅÆ?¨–L"ð²?¯ôŠýHÁ?'Õ‹\ ³
?¤"O¦pÖ?íçî䑫\?³UÒ÷mN?»hÿº±{?Ó¦àž?±Ž9"€›?›7}º•sb?êlÐxÖ9½?¤"ÕðEÖ?"{ 'ÉÈ?'¯YÃ##á?rªdfa¶?k£ÅÉ?ï>Î2¥ŠG?" þ°uD4FGL J1839.0-1502?èø×0˜À‡zA¾	À9–ä+Ž#À;4Á5¿Õ@Ÿ?´öÂ?@›:Æ¥k_?ÉCáè<ë?ÓKaþ!Ùo@ÊôW@eÜRÑ´?ïÿHë+\¥¿Ý2/'"š¿é(¯ Ä¿â7wÀÖÊR¿ï®+ALP'¿ïÿø]ˆòUNASNone?ؒ|ä³íu?ÆBý£°Õ?™]†a:§¶?"è—­ä{m?âëÕZœ4?ÆH©3ÂÙ?Ьw$åC?Á_¹¤æ?£ƒ³)ù$3?¨•öªf?æ¹î'Íû?ÂQç79F?ÒhòÌ!?¬TUì*RE?ÂÏ '·4?¡qŠôûœ?âDãÐÌð?¬à6g¤ÂÕ?ҙÍTŠn?¬¾ªÞ,òü?¸d_2þf´?ŸMºy¤?㦍o•íô?±¦ÈNT‹24FGL J1840.4-1705¿ç±€x‹WÀ]^^Z(kÀ:NH;Øô"À;¸©Þ‹;2@ ‰iw½Ñ²@½D™?ÒYª–A ?Ì'—ÉŠÍú?üö¡ÍDÁÑ@xœHöi?ïíTa$X¿îL'\f2?Ùþb;^zà¿å°ý-½¨m¿ìêÛ@-¹?Ä=må™!UNASNone?¶Äð*åÛ?¬ì¶OW&$?¬©å?õÈÙ?ªyì^*hé?ë\æ¤ø?µ`Î	H?ζLÂk¶'?Á÷"T2Š/?æ³Åè.2?›Šè<})?çË715Ðê?Á¿+¶Í!·?Ý˚Š¥X?¯7žÀµº??·óGZJZ?›èTç.?Üp¨¤È?­éöµê<?ÑØvÒ«?°–¼|ÆF…?ªëšZ|(²?¡ç"PT/?åenç´?³l9îŒ$4FGL J1840.4-1139¿èà½F¿NÀlÀóz¶À:™[†8"À;ø÷§kê4@ËK;½›W@'Wɱh?͝Çüƒs½?ëkö}ö%@œ(²¦°Ù?þ8›7(‹:¿ïým´8Q?ïÿñ¢o+1?ÝKáÕÈt¿çW½@½µX¿í¬¾¿ÃÏοïµ{A¿½ñUNASNone?îúSÝð?z3rÜ}¥"?á…/Ï?ɧ‡¤3?Üm¾)/t?ÈàÞËI;?žAÉnlQ?§9
î¾û3?ÝÈR{Ó?ÏÉàC³k?à)Íä-4?ÍøÑÊĞc?¹ÏÊü—Nƒ?˜ŸiB]S?â•)¦¥ðX?²é=T´f)?Ôa¹óŽK°?°"Êm€H?•Â×Ý©)?‡˜Œ¸_¯Ò?꟭'Ì?´(
'Žy?ÂÈð¢US­?²b›$NZ?4FGL J1841.6+7113?ɺ®š»5@:Z–=Ć­À;tµcú{\À<ö«Yµ}ü@ ךÊF4Ã?ÿ׉¤Y=?Â$$wƒš)¿©CH ¢"F?ççf¬ƒ¨?ÿ¸Bi\ ¿ïìÎ?=­‹?ïüZžÜúl¿ç÷>Ælª¿ÊkÒ6?è¿à@H»ÊF¿æ&ÙRíÞUNASNone?ïßöîͺ?hc>bž²*?JK²';þô?J2yk'-ÿ?iv$Ž–Eç?ehVævo?¨¨.l?ˆa"Ýl#{?JïþúUÃ?[XæÅý?ˆ¬•õ"¿ï?†ceA6'M?îH+–ËX.?ÎAk²?t5š6BL¸?eVç·(…?¨ö"L'3ˆ?‹±
ig†?îÔ(Y½ÁÁ?ˆPGÙyÃ?ƒØ¡Á§–X?uiÐـŽ?›Ž£çsüº?†5kRPW4FGL J1842.1+2737?ì[‹cmZ@,+ææS†À:K½R†À<ˆd•y@Èü¶õJ?ü…Ö|?Ķ"‹ë[-?ä†ü^	öy@eê«%)@ÔCíë€l?æÀv蔩p¿¾z% x…ù¿©½XÚ©¿â§ÿ¸ÝW¿î͐ ôí'¿ïžÏÎß̄UNASNone3FGL J1842.2+2742?¯¶þËï?°†gHOԞ?ì}¼.xÞÍ?·ÀQ< ?¨m>Mf"F?¨Jóƒ[ß?·ÅMS߇?ºÉÀJS…Á?éo¥Y_?ÆRcÆ×K?ÀšÀªpÂ?½…±?Äç¡×¼Ni?«cã‡Úˆ?ç®!ZÕÆ?¯6C¡µ"6?¸¿±yÞÔù?›µmp¦?Ðí&@1ð?¯€²–‰?âCÈÁe?´þ!¢…û?Å´±<–Š?¥"0÷Ž4FGL J1842.2-0328¿ëïäŒå‰»?Ý:
b>8 À8hÞ4Ô#À9¨XŠÑ @Å÷ùñÉ@Òa¤_Æ9?õ¥ouÙ ñ?Émµ$ºt†@5%1?ûrEî¿ìxÄ'6N?íÿ*¿åc'K¯¿ì'<ðKW¿ä • ãû=¿ïÿÿÊPËUNASNone?Ó¡s¯-7Z?×Tø*?•Ú2%dUN?­Ë™Ò	%¼?å€t—>A¨?×0‹v)òð?§2ç|ÑÕ?±ª¸íSA¡?Ák ±"L?ÄÂ+Qn™µ?ê2	[ú~?Å¢ãc'~t?¹ÃqÆíÝ6?Ÿ°ãAÉ>?Én¡'ã]Õ?±àS®>?ækéfilã?²6xš"0?•,»Eêùs?•Æ
¿Q§?øÓÚÄ?Ï?–x ˜|Ë?ï¶Öe—5?ŸvvStk4FGL J1843.3-1242¿Ñ¢çöô¿ÀÿdIU´gÀ9Ñ{m^¨,À;pSÒ+í@Ž•¯4@£þwiÄ?Ì¨¯â?ÒåAbËÒ@'ö¿ž(@#V/ŒŠ'?ï;Eñ{ؾ?î/¥>éIÛ¿á<DSìç¿å«LŸjéٿ퐩e¿wz¿âÜþ=ˆ ËUNASNone?ÄæªÝV?¸ôä¿'?Àç'L]«ê?·/–näIp?挝'1?"?ÁÒ·ÅD¿–?Ð|ÇZ	?Âz\†iÎ?§'ßÙ|ß5?ªF›¢4¨ö?惔"…?ÃÒC"£Q?תbú—27?³T~<?ÁdÞÚZ¨?¡ÿzçUÞË?ߣ.û u?³F#ÎM?ÖSGŽAÞþ?®(¾#;<Ñ?þI†öò?¨ùE*`?ß͓®B¨?°mØDôd4FGL J1843.7-0326¿èÕʱ¶?¹hšY³À8/r&À9|_æ¤í@W­»åt@ºd<Àz¯?欂ªiËv?¾²pK˜?ûV'QúŸ?ð•˜/âè¿mÜ	‰IGû¿Í—Ðk½¾<¿äÉh^Ž*Ñ¿éªÃø贊¿íþVèD!˜?ÜõÇb)ÀÄUNASNone3FGL J1843.7-0322?z(ä[rºò?¦Z§éMÅ·?"jñ'/0? ï4¯²´?ïzq@]È?¬§ؙW?œˆÉ"X7?£«¹õé%?«7Œog1?³%nÀ`Ôâ?íh@ïöΤ?´ÈŒ¤ZÕk?´¸Q`²1Â?—Cè(±k?ÅèL©?¬´f$ap?è%1Ù֏‡?®‹±þµ3?j1ùMp¬Å?`ÒJÿ
?w£µ"X]C?'˜R–¢Ç<?ﶆ›©Þ™?ƒy`—4FGL J1844.7-2110?édg
{.À +éȆ/À:Wꢠ©À;³§¬_o@W欜֐@Ov¼Ï)?ÊY&âÂØW?ÌÒ÷_Ÿù?ÿ'zH›zD@0‹1vðw¿×7¡2À?ïû@>Æå¿ç¦âøˆ<z¿â¯Dü‰Rú¿êàx`cíæ¿ï÷#b…±/UNASNone?ݝy¾‹?ÄxôFõxi?µœUÎhË?¸Ãêl¿Üë?Üû؀ì'?Å't û?èi4+‡`Ç?Ɓ8¸Æ?€N‡–î?ƒßÑý"Æ?ÍVF؀úå?Æ- Ô}³?â®=žÿw?±ë,Vܑ?²å;d%ø†?˜ übQ?Õê5è÷'Ä?®–À|$}1?êniªON?¡ÙÈ7«?¤×'5iÁœ?Œ|X0¨¹è?ŒeËüR`?ž6^|Õtª4FGL J1844.8-0957¿ÏIµ%TVÀ‡«¨À9€_7ûÿÀ;Íì‡}7@Á¡w‰yf@Ö$o…Ê?ÌY{ÜÅ=a?Ôn›¿
Çi@tòñ#Ä*@¦Ý>ßå?ïæÍ)Á¿ÞôC~"ë7¿ácÍ.ò\¿éÐÚB×%¿ã#¡?€H¿ïü¯ž=Ã/UNASNone?º,[HÇ?ª!?x°d(?"×›'Ö§?s<ÕVA?ìÂÂû˜2?­YuL+Ø?Ňè|â¦
?º+8B^ÉA?›·ÿ,n¦? ÞCÞi(?éÀEçgS?»VHc²Š?ÈesqÞü?¤—p¹¹¡ç?¿[îÂfm?ñ2ä"Ư?åû%KG"1?©¯NÊoGM?ÁÙ/"ôž'?žÿ"¤®#¦?­ƒk]ëÐ?'H}Áïÿ·?鱃TùŸ?¢ÃLðZ7‰4FGL J1845.0+0159¿êÝТ'²<@¡®ÁIÀ:Œ°càz)À<:.›ô½­@žªÂ`ã?÷}}8Ð+?ÑüU›½á"?ïÿ?`h¤@¤Æ†"Ä?ûïm£Çoì?é|Ÿ5åÀ¿ïø''ì×.?ïÙ8`C·¿Üê_d"(¿ïþß~«+½?ï 'àðUNASNone?׋[3(#?ÊT)ïàº?Ãei&æq?¿uw	ƒV?ÞÁð9"Τ?ʜɦ"P?Í"R'Eã?δ"ó[õ~?É|8QË:&?͆b«$:?âX]eƒ_þ?Ñ0áIŠ?×*¥ò'<\?°¯׿*U?Ôd}!¸1*?²ªoŸb"?ÔpÜ붒z?¬«ðd·—Ù?ÍA{ùÙ?¸'†)­™?ʀ;ýg‰˜?Ã(-?â'>¤Ÿ%?ÆÔ
·¯4FGL J1845.8-2521¿ïܲMùÔÀ$=:uFÔÀ9"Bþ'Q~À;Ì"ð½m@Sj¯÷)@DàÑ?º×ý­j[é?҂A©¨…@Í%îÇÉ?ô@gÌm‰?ïðcu^P¿àšdÃÎ÷¿ßn{=Ž¿â"º?+Žú¿ïšˆ!L*ü¿ï›¡æoUNASNone3FGL J1845.5-2524?·h ¿ÅI›?°®B­÷?Ùú¿
›¦?ȋù$eÓ?àŒbûˆú?ÈY[ëF
?ªùò.ÌüZ?²[±Z,i·?â7<?β5
"Žb?؀‡Kè;?ÍÈ–sŠ?ÁuÌØêv?¦¿ ¹mÐ?âÓ6~GÓ?´4mU?џ&Ž0Ÿ?­µfxÇc^?®þÂH<1²?Œç…-Ç$Ø?àds4 ŸJ?¸Dbð#?ÛWAM·;6?·_3Weç¢4FGL J1846.0+0507?åÿ!5"Ç%@HüBÜ£À:8ÓMŽÀ<Æ
:ìe@fþ¥7§?ûIR>'5G?Ì5?ÒÓÍ?ã'-Ê=¦T@°—"ìck@`{—%  ?îž›aö¿ì´=õ.æ?Ã:öËù¾¿ÖÿÊ{
èK¿î'Ó¹PF¿âúy]¹ïzUNASNone?»EoD\?°Ÿ‡¥ÁÀl?ÐK5•tˆD?Áíi(úÉ?äw\•ÓR?øKhñôc?УbpƒK8?ÊóCA?Æjà‹FX?ÆɁVÝž?â–¤ìÄ??˪ƒüœb%?Ú©%ü‡¦?®òÌ»nà¼?ÍÂjˍô?«
ÀD'Ù+?ÖuÏ΅±`?¬9Aʖv-?Ü*™¼Šp;?°I"Ëñã?ŵ֩tî°?°ÒéœC¶›?Øúzî»m?²Ùåh:vo4FGL J1846.9-0247c?µ 7ÿ†ï"¿Ñ÷u¢™r'À8Ž€µÀ9þ±¨ó@ Ë´Hòb@? äçuÅ?ÊӚFgÃ^?Ú1à!é3á@LfÓs¯û@
5^†ž¿ã€¿ð©K?í§\€3—¿âp*ՖŸê¿égDýàëé¿ïþ Eð¥?ïiQ;UNASNone2FGL J1847.2-02368?°|üó­Ç?¹¡=ýÆ?®V‡?}Õ?±hæ¡Æ>?ì
÷ïæf
?¿HT¨÷Þ¨?«Gs$œZ?¯	nUS\?Ëüüå?Å©,+æ?çG¼aTNö?Ƃÿ•Å[d?´Ç|g"³ƒ?šI ¿:áj?È=c]Ò?9?§å•ª|a?çW·›§Â?«|/­ß3?Š+ÞÞ??~¬¹Šy¤?·È s«‰‰?¥¹[Có¸?ìˆÃE{V?¦Ùñ'·*4FGL J1847.0-0625¿ñ""(–D¿ÿ-O#SÂÀ:GwÀ*ýÛÀ;Õ+y*ŽI@k÷τâþ@eXê|àü?ÏÈ÷ê‡É?àþ_o×(@¨¯bk/@Æi/œY¿ïýêªr/?ï¿©~+V¿ÏåH U5¿Û¯Cdƒ¸1¿ïiÿºùf?·Qx!$UNASNone?Ð8«ÎAª¢?¿*šmv¥?Án¯¶Ùm?¹(7¦Ã?ã‡þ+Z´T?Ã\aªï¥Œ?қêo8H˜?Ǜ#Ø#?¦ùÇ'éÌ?®åWÎØ]®?åBnUë½?Èï¨K?Ü8"'̦?±³§Ê¡y°?ËÇY8Ý?«‰oäXì?ÖCyÁ:–ê?¯j»8ˆH¶?ã•}fñ¹?¬èà |?·‰³­vq–?ž23}W§?Òò˜F¾ñz?­Â[5»p"4FGL J1847.2-0141?ìŽÔá0:?Ē®Bóð}À7å·lé7À9|¡|¼ê@Œè¹èC¡@ #¦Î5ƒ?Á!¯}0­G?Ö92¼î¥@}¶åû@f·Œž´a?±öí ™¿½?¦´	\u¿á ÔV.	ÿ¿é&Ébµþ¿î"]à…ç5¿ï¥íš¢®UNASNone?r µG¤â?p–Áì
©½?Òʬÿ_[Ý?ËS,~´"?æv>åÂÈ?Ëe‰'âê?ŒWQ2­ˆ¨?"@y")ú?Ôۂ¡±ö?ʞ§Ã÷A?å áj\'ã?ʋÕ}\¿?Ÿ~Ý;Nä?Š½"Ôs‹?Ýì3Àn¹]?¹&̯)w?à
ï5ð Ú?¸ÕüŠÏo?R5ë ?Cs"ÂU¡Þ?À½­	ENG?¨YR g?ëÇyÈ# î?¨§NmÎ4FGL J1847.2-0200c?çf¥v»?Z8ž'6§À8`§GØæÀ9³a°ôÿò@ †l(T@å eÑ1?Û'¾Anµ?ä'ô>UÑ@ŠÎ$»¡+@›¶‹lÛ ?í")à¤&¿ãւN8ó¿æ›»øi3¿è$nß±«ß¿êLÆ¢fFÜ¿Úöüᒁ¢UNASNone<?'HZyï£o?¨ewÙù¬ã?ºýàg?ÃÁŸè£X7?ìMA!?Åf`'Àg.?"›Šif¢{?œî0e­í‹?ÁáŒäWF?ÃD@m.!?ëëI{µ?ÃJƒ+ÛA3?ºÏ$Oõ?šWÁVûT€?Æß_zôÑü?ª"Ñk¹.?çî<¸ÌÞ?­+›CKF?bìÝÅæ—Ó?S&à"¼l!?¬ï#)Áá?¤ÎÓýÊú?î ï¨íJ?¤ÞoðéÖ±4FGL J1847.7-0125?ï}¤#=ûA?ła€"¥À9PþöÅÀ:z¶ƒn@!ê
¬»à@@Ca~ ?Ï<â()?¸.žp?ïÍ4›èÿ2?û;Tiä ?¯òlÄyl(¿Ú|#¼ó'¿âð|iÝê,¿êSb}¤¿àµfÿ"s¿ß½×üÖªÇUNASNone?ƒ@gbà¬ó?ût÷Îãˆ?OðÑû•HK?[M!®v¿ó?ï«-õ—ú?ƒéloû?¡ßÁclc?¬áèè"/?–äÔ-etÖ?©­)¥ö'?î*ÝH^)?³D)¥qVY?¾ÍCRã§?Ÿ›<ÁWU?°a´hٖ¿?–š°3Ö@5?ê!£P³?¢÷w¨h¨?,ÅÚzF'?r
cÐeJr?slÚ"ÄM?n»ƒ§G#?ï"tºáÑ]?ywÁ•eæ4FGL J1847.7+3543¿èEéUˆ#@0!†¹ÃÍÀ;Ÿ¼
éÿÀ<Ͻ¥œà@!j\‹ò?ñ•:uFÔ?ÞÆÀQ>a?ì¯:€.Ž‰@P¾yLòø@Ú%ñ]É?ésÌ`@\'¿ð?í—ß…65?ïÿû˜'2¿ÞÀÝ`í²¿ïþâ~dßÔUNASNone?íØ|`"©‰?»¬ÂjL?Œ˜ÝœIÞ?'Ž¶ªÇ[K?«R´ŽTö?¹ÕOëGEg?쯀[ûÈÁ?Á%ŸíW?•®FŸ@Ä?¯›ÎžJŸ?µkxQ¹?»3ª'27B?ëĝßçª?¤xr3ÝG?'²Ç¦ë@ƒ?çÀA3'7?½neGEò?£gC˜4?ëœz(…–?·÷L-Ð?†@Ðj¦*{?"!ÂoïcÏ?À*
WAW?·=;bqå4FGL J1847.7-3433?ÜyDW¦b³À,˜â~ù˜À;<Ž%ÈÀ<£yv
£W@‰nMægÓ@.Qúž—/?Ïê¯ iú?àh…à19@MZ%æC–@L¡°ƒ•?ïûñ}†=œ?ß8KgÝ_¿ÑúÍ%¸ m¿ã˜àkæ(¿ïìÇÿ]˜·¿ïÿàöO}UNASNone?ê
˜ÙCÉ?¾'yŸ÷Q¬?Áûz£7R?»6%ìÒ?§:$…>æ%?¢5.È
›?ãà`ÅÎÊ?Èè
ò»ìI?̀;q?'næŠ{?Ãýï­5»P?»¼"À°u?âŸ`h¿ƒ½?´V—iÙ±ð?Îp½ÂÙº?±fúŒzú?ÇÀšûN?¥ôÌ¥að?ޏ—öCà|?°¯èºâ?ÔT,â5"ˆ?²ÑhYÿ?Ê8vO
5÷?§&rŸæ!4FGL J1848.2-0016?ã‹IJTj™?â™X {öÀ9@©-À:…! 8B@l¦Ð
ôà@Ó!_Ìr?ÉA¥Ãt?ÑâÊe€@XQeMa³?ñ´FÁZ}пïùÚí!+?ïðBRŠçO¿äg¿Sg†¿å`5•
Bß¿î/¢ŸÒ˜¿¿ïÿÍui8©UNASNone?¾+óÈèé?µ*³©¬´?ÅÚÐÞ4¬?¿˜B9n¤?æù#ÍOU¸?Ä©Gëºü?–¬ÿ7Á™"? M	eá~
?Јìu¥ ?Ʋpû..?ç‹ c?ÆÅ¢%2©û?ºëÄš_\?˜—ë1k²W?ÉKú€xª?¨Š8°¤±}?æOˆÞΉ?ªi¸¿Na?_©K'ޏ?yµl7Îò4?ʋ¨¶ô?±¯¥=RÌQ?èÚ>Ë£;N?²0yp''4FGL J1848.7-6307?ìފíâÐÀ7³c€ßÀ;Ã2ú(OªÀ<ààðp@@!›?p-d'?ýÎÇä/¿á?ÐÖ€Ú?ªó/bN?מ§Šóäi?ùÅ¡²:$?ïÿùµc#¼¿ïÿùµc#¼?ïÿN>úg¿Ôú­ÛšðÝ¿æÏW´ü¿ÚTË^b¶ÙUNASNone?ï¨
¹5-ö?•Ënâ?$gTI:Û?+ªÍçjA?…ªôa—-?êK1o€[?ïŒ"'¤?ž)FF´O?`‹ô7"5?t]LAC?\îèÃdâ?œ(°•Íº?íÙ,ŒwE?•ø/€É?m¯fa¬??bQöpà¦ñ?²£»ka8t?•¥üÞ@r?ì^qc˜?¥T‰"W%?~
·Q³€?zŽ¡Ëêx?».9ò ?¤à žØ4FGL J1849.0-1826¿ìâÝK[YSÀ-s!_ÌÀ:hÒlHþwÀ;ä"îA'›@ÇZeý
@Ïw¡øì?Ïz!™­»?ÖÔx<ҙ@@¸â4=@In+ߤ?èÃêXÎÎ?ïû³4uR'¿à¶e)O…¿è@Åø50¿ê3^1
¿¿ïÿ¶>@£UNASNone?Î	6ÍG¤Í?¼Ù
u&=?»;'Àn3}?´•±ÝíÒ
?å@ P]?Á¸é÷PÔÏ?ÙÌ_íkÊ?É·ŸÜE¶? 
,Þõ?¥Ô§	ÔF¬?â`GM
?É?‡hì*=?ßÃoÕ'Ë?²7o?ÂZ£9ä?¢6Gõµ[C?× ;C?®Y'ôâ´?â܃AÙÿ?¯D¼¹es?µK!Z¦ãÏ?Ÿáz:k£ê?Ôô1%¢HÒ?­e÷æp4FGL J1849.4-0117?﹗S¡ÆA¿Â¨†z'À8T‰.‹CÀ9ž¡´N`@¿Eß]H0@'–é»ñ?ä@¯¸k?·ùf³¾3?ùg£áñø@û÷­K'F?ì"\
G`¿ážä'åp2¿è°‡A}Mß¿æ†o»y¾2¿æċë[-M¿íëÏÇSHUNASNone3FGL J1849.5-0124c?'e `ã(^?«t¯h‹¤a?wµ8–èË? Ï}·#?ïEl‹ÌÜì?°m
ô3Щ?°'¡8lD/?°—"3'Ÿ?žS.®©?«¤¸'?ìý©@?µ1ŗ/ÆÑ?»u‹åéh?¡+cyñàR?·ÚöfJì?£ªæÊÁ\?é•ïÁ¹u?¨Êle†x9?˜ùgµþ ç?‰ñ;Ӎ'?gbZblOd?n["z"‰?ï Òg힪?‹ì_˜€ùF4FGL J1849.8-0952?×¾là†›™ÀŽÏÃøÀ:fc$'†€À;ʺà;>š@ƒ‹û¡K•@|{*BÊ?؇Ï!Éf?ï."²‡§@
†Ã%"?ùœbCÁö°?îxËrK!¿Ç<™"ü.d¿æэ'Mš¾¿ï?ërªAˆ?àc¯ga8)¿å­j0öBUNASNone?ÕdÆÍx?-?޳v˖?½fV_0qú?·$x"Xç?á ÑÍ]Ò+?Ç)Q0*Wþ?Ç"Ýù_L?ÄH!
Ÿ?³RނÝx?»	ub¬q?çÒÂø-ì~?Åõ«zU?ØF'›Òhc?«áÚ6Nx¬?Ée:A_ú?¨Š—|5mý?Û,»ÇçŸ?­Á†.[å?Ë+î¥#?ºq«¼"áR?˗Èd'?Æ
/?âOxˆ¿ý­?ŪÞ; ªt4FGL J1850.2-0201?í@²3¿åg|`£®ÆÀ8ïcF÷5VÀ:#Mçê_…@ ´nÒñ	@ñhr° Å?ÆÎ8‡°ãã?‹«íë;³ñ?Ðô:$/³?þÈÍK¢Àµ?ÚºÔè$A(?ևÊ#ÐÔ¿éJÙ!ï¾ê¿éì°Ý­ð"¿ÝõÝ%O›¿áÛÇqC9;UNASNone?Š™Y™Öž?ÖoÒþ›p?'Ç;«°	?¢Œl%;?ïJ}ªéåb?¤qj5Y(…?±#jÀTLb?±ßÖxJä?á·}lhg?Ÿ·W|zõ?ídÉÿÄÓ?³e¤Úhk?¸§‹öÛMã?šÑ,º?±À˜ûxòþ?˜§mÅ)?ê²ûaµwã?¢ÀYÞ·s?¦Ž·½«=÷?"áŬù¢?ƒêÙnG'?w)¤ÁÛt?îGjL¿"?•¿'ҏ34FGL J1850.7-3126¿ØÀ©ëmÄ À+@y€õ]æÀ:—žã…uöÀ<:g;x|@ùª&ڊP@ýã$ýæJ?Ò¡]•Ç?äÙ=ôWU@y…'Î?ú‹šZ‰¹R?ïêR^œ˜}¿·*1¬ËOŸ¿æˆ­'f¿çZ.I¿f³¿ïÿñ¢o+1?ê©}'QýUNASNone?᤟‰,¶?Æ¹Ö žOú?Õ\$ۋM'?Ç<GE#ÉÊ?½jpI¹dG?µÂÕT© ?Ú¸€4H.?ѵ0±Ù›?ۃ,êƒ`;?Ò7˜Ý?È¥Âhã{?À9'ñáïP?ÖÅÌ{S¸?²
øcmhö?ÕúJ$è¼?³‡Ô2ž\?Ó?é_ù'‹?¯6Wƒ·¨'?º'bÁ§5? µPÞ³ÕR?äaq@¦?¹,zª|a9?Й2˜Nzå?µÀ=÷è?=4FGL J1850.8-1105¿áÜÝIwîÀ•?9ѲæÀ:yx˜˜ÚÀ<"u]@–ú©T@0#Á¦(?Ѹ:#gc<?éj܂Luú@þ"'Ùc´?üý"åø?ïüB"ßοéwKáâ8¿É*QwÁØ}¿èÑþåxÀ¿ì»4SÄ£3¿ïЋ¾dª$UNASNone?šú¦›?"mZ±î?ʅhû}Ü4?ÂtŽƒ}?莍ëë°Ú?±úLênê?µ6&!ÆD)?µøO§Æ?ÈPû-n6«?ǬÎm8Ž?çDüpk©Ð?Æø+²¡j?É÷PÿÎ6?¨B7]J¿V?Ü]"¼¶_?´XŸ‰_Ì?Ö÷ú]\H?°ˆÕoÄ?¬'Ô ?ûË?ވÙùA?â*ÛÙq?¶@&PäH£?Ø]&@M¥?µ%õ¤gþp4FGL J1851.0-3003?é°ùærÀ*BÀð¸À:ö2÷¤À<;ê'Ù²@Ú<ü@:Ü$X¤Ý?ÁY«'zC=¿°<°	š?ò1r¹[@€
Y]¿?Ð=û"ˆý¿â#¸¿ëH¶‡D¿Õ][$éÄ¿ïÿü9¡â=?ïÿì»"UNASNone?î9"E¯á?¦U¶Êü?Šb±k"4?"o¿éo´Ð?¥Î€áÝ#?£ÄõÜÞ(?îÁhÆ'Z?¬ÞhÿÅ?b!¢ÓëÂd?s	¹x&?¢ÇYr=?¬8¿Ï?xÐ?êñÒX‡°Á?¨Ì?¿BD¬?™P¢6j ?ˆ±ÈP̓m?Á¢Wèü?¦/²å¨0H?í_)ݚÝ? h}_Lq?€aߍi4?sgîŽ\ô?µðåµ!{ç?Ÿ<ò±æÜ4FGL J1851.5+0718¿È‹)iZâ@
i‰¡ÑÀ9"5´í³À:ÆÃhŸý@°¯þ4ù²@ýˆ ËQ£?Àdlü'œþ?É":·¶æ@½[û©Y*?ùPx–Ó?íU]T™à¿âÄÜ=ƒN¿èº«'OP¿á`‰½®vË¿ïü¤ávR¿ïÿùµc#¼UNASNone?ÓñÇêx/s?Áu¸Î}Î5?Ϛ^0òÁ?Á_əê'?Ü@éfoW-?ÃãUDÉe¿?µýŽV\³?³Mɘx—?ÔWÜL´—?Ç/ŒéW¾¸?ãËGT?Æଶ'Þ?Ð/!½o¼?ªîƒ"Ÿ?ÆÁæl±?¦k$?÷½?â8<u†Bµ?­ÑO^£?Ÿ84G?†8AÃðW?ÇwWú?°8ahUK?é(}¦.Ú¨?±›ÑTYF%4FGL J1851.9-1522?퟈—HmÀ6F(}‰À:zà,À;ä€Ø´5@Vœ.t\ž@ã7!Õ<Þ?Õ\ôb=ú?íþdŸfã@7Œ†‹ŸÜ?ýkûägs,?ïï˜p"¿Ñ7è‰ø<¿èj&Ìóc¿ërH½3«¿ïÿÚÁ,/´¿ä$ð_µUNASNone?Ô>œÀ}Ù?Å£—ã2Ô×?¾yó`ÓÆx?¶†«uš#C?â³Å…HD?Çhÿ1æ"?À<©³Æuõ?Ã/X°£b?Øà[ǧ¢?њO…'?ßO_d?Ïóa?ÄÛª?՘΅?¬"":ÓüS?Нô`=?¯SS4%c?ÚEs-ñ¦?°Ö›I<t?¡%R'—ž?Š¬ât2¯?ç{|¹Ê–?¶_
ìlsô?ÍÈ¥‰x/Â?´Žd%´4FGL J1852.6+0203¿îʽLŸ?åcl2š‡À8
 yóÀ9îäùê<I@^ô­™Ö@¬À½ÊÑ?Àâ3{ØhŒ?ÃK¤n3å@o‹XŽ6?ó,c8¯ý?ã¥üH»Zµ?Ír!²lN¿æv÷"‹Æ¿è¸€å¿ê–ß~*R¿äîDنUNASNone3FGL J1852.8+0158?—eá×Xÿ?'™›[Nw?ÀÎ\ýÊ?ÁóÞç´?ë@Ì=­ÿ½?Áä?ܯcÊ?‹ª
,!?'Þùµ·DÅ?Å"ዃŠQ?À_M‡¼ÚÜ?êHŸ,ömK?Àcž<Üé?´Lå8ú'N?•½X÷La?Ã|›Œ"܂?¬ÐvØÉܦ?è—<u×ö–?®øÁ¹#$q?rh¾ðkå?aF㋠'¿?À¬ZæVµ3?¤E¹'µ¬?ë°ȊCÛ?¤¿sЎˆ4FGL J1852.6-1159¿íÇÄQþûHÀ΢(´TÀ9çrüvބÀ;p££×e@h¿:­@Zñ£EêÆ?ÉSme^(ª?Åö/‡,.²?ý[ö Û­?øäC%ï}Ò?ïÜ5?ÒÓÍ¿´¨JŒk2Ô¿èûù`(´ª¿âwÆ´{G¿é¬lÚô­¼¿ïÿ¦<ådUNASNone?Ëi<M«?º8¶Åíþq?›{P¥–£?"û"'´?èIßóHá?»—$ÄZ¶?Ç!$"X¸?»ïÏЗ
? _Ùo;Å?£
B/4š™?é1Á`­?½À#ò–#¯?Ö<•òƒ?­ì¾ßU?³Y'ÛÏá?"2ÉèÈ?âvvÜZ?­à½b]Ëy?ÈõÚ)¦%?£»j˂ì?½Î•lÙW#?žÎ€­a§?æ¶ÇûKÙ?ª^Ãt4FGL J1853.2-0922c?íó³&;0¶À¬¦¡¿ØÉÀ9ËÇ;"TÀ;MC0×8a@nLÂ{e&@®qÛ®ï?Ò3Ȅh¯í?Óø[{¦¿r@j ÒH7?ú¥mL¿ïÿÈ‹ñ:?ïÿY¢Ò1¿î2ái<¼¿ÁÀÒº[Ü¿éâÅA¾q¿ïüí'hr°UNASNone!?â'S"(Ù?ɑÊrg<?¿¯ŽÁÎb?½æÛ#Æ?Òïu(rª?ÈIdßȒ?Éۗµ0ú?Ƽ¡	«>?Åõ
®?Çú=€›¯d?äÖш?Ì«"êx?Ñ> u¿[#?ª†›gsRÔ?Åj>:Z­1?¥´;äB§?â`6‰§"?¬ß8¾ˆ²ò?ÐÑ[ùš»ø?¶'¶`‹
1?ÖÄ3i!å?ÁÇ"{&?ØjpI"#?½¯‹€Œ¨4FGL J1853.3-2447¿ÌyBƒž=À&Û¦&oÖRÀ9ýìgpRÀ;µt1*Dw@ÜÓò0±@Ôa0œþ?Æ\ÜdokH?ÅҁGRÐ?ø8¸®1×@Ÿä6v?íê­ÞJ"¹?çßùÀë-¿éN¯{㦿ç–j€˜A¿ãi!—)|ѿ䍍â?UNASNone?àºT-¿|?Èr }íÖ?®aǍeE?¨vʦX›W?Ú¿²ß{!?ɠݼK?ìÂx¤«/?¸™ÀáXº±?éÙT¥?–XÐU·–?ºÿ±Ä•QY?¶µq÷3€J?âãt˜¢5Q?³•Ú¾½?®MxÚ91?'Ú×MÆ?Öví N7?±Ù"u6ØÎ?çjª{.rM?¦W'ÌeÔ?«"Ù
\œÖ?•$K6.E?Ëp_Ïï˜?¤6ðîåÉ54FGL J1853.6-0620¿ç Gñä¼áÀ*èáÖIÀ9ÞŸ]'ùÀ;6â¿}Xñ@Ô¹¤{õÅ@ÁŒý©äj?Äá…@œ'h?Àí·(Ùº?øLZ·»+@ÿµ$¿ïþ;?ïÄÒݲù¿è‰áØT¿ß¥ý THØ¿ïýÈ[fX?ïB€®IUNASNone?拺ÃÿGá?Áë|½X?'Ï͑9Å?'wMšÙ‡3?Ñ»žïì£?ÁÊùúí;«?á<Éր´?Ζ»A
ƒ´?\SZŽ? ŒÅ	<¸?Üö£ÏØ*%?ÎJÞ¹ÒN}?ÙR¤¥Å!?±ˆú1¦?µš'z×5t?™­O
eš?à£]]B?°õꥍ½"?å»ô.nx?¶ªØ"ú?¡¸;t­t;?ÉJ2‹­Þ?ÒQe
t‰?µÝ¸'¯4FGL J1853.8-1107¿Ò
Z
´ëÒÀT#;z*À:TóRr"›À;‰¼9Ҏ@méLµ:_@¼7£~ö@æ|­_I?ç!J}|­{@'«¹VÎC@%ÎÚÄU?Ñ@|g¯'?ï{ÝáÈ"¿çÛ'£²ø¿ïà.ʖ<?í®ñðs¿Þ!§ÚúâàUNASNone?ä_LH™W9?Ïò½ðl4à?Ðt'…É)*?ÐmüÊé×?»3S¤¡ˆ?¼üI äÈl?Ö2£Ø
¿á?Ô u÷š@?¸ÎӁÎё?ȍ"m¤A?áÌÓ£¿EÝ?Ó»ågÊ?Øi]ˆ›\T?¯±g@™Tã?Ä=–÷¨ ?¨€Øs1B?ݒƒ«èÏ\?¯hæä}-?ê1>Æëf?ӚFwÌaï?|ÛÃ]þË?®Žk//ÙJ?Æà\èébq?ÓG¦Í(ÏT4FGL J1854.3-3640?¶{¼šÇ×À0ZÅ;ËÀ:ÈPÓW*‰À<SAÞËÓ@$cb@.ø; ‡?Ó"ë|æ/Ÿ?ÔKÖãQª@yÀÌäJ@WIí	?Ðe0pá¬?ïîh(†¿á…ô¡'-¿Í']êâ¿îuLþ`m©¿ïüþy×ÝUNASNone?ìk«}"ŠG?­ûE®¼Lõ?©ß(ã—Yj?£ðPQÌG?¯fC0&?£Y'­ÈÚõ?ì…:.‡?µ0"~ê?¢<+Ý|Ÿ¯?§'å²ÏÈx?²¸Íw;?­º©9uO?éHIiSßR?¨b®š
dr?²K묹TÒ?˜'‡?¿?Á¸ä"SØN?¢²-#o&"?ç6ú÷+{É?«rfçÅÅ-?·ÀèÜxw?¤´üúò?ÇC ãÔ¡?¥ÇDMF›w4FGL J1854.7+0153¿ìñԜW—Ÿ?¾·¨£L˶À7ù$(Ô4 À9ßc¨F@ÙqóbbÌ@3‹Ë{?À^®÷yɛ?Íà*w¢Ï@\E˼+•?áh­éæ@Å?æØq
"=¿ç'ö?p¿å/< B¿å»bó_¿ê†È½¯#¿ðUNASNone?ÑI¶>?Öª'µ:?À¬_'¡?Â}‰ú´y?ã{Õ<ž?Ô°"?"j'‡#X˜?"•Õº#c?ȼѾÞ/?ÈùHK§??é!Uó»?ÈÉP	¹wc?³'ÞyKjá?œ¦[^º²Å?Ð3»o*DÓ?±jö ?åsÆyAp:?±gšÞc\?Ÿ$µ"¿?ûÚÁ-?¸#"/HD¨?¦•×èb2ñ?ìú¸ ðá¾?¦˜ˆ(Xl4FGL J1854.9+4054¿ÀÌ&Vçÿ@0Â!x÷À;>D¬Ø:¿À<jV´A»Œ@þD<ÅÙ@Ñ¢£Y?É[~€äl¿šGÚ<Õ|?ÓO*_¥,?úZu—[Ѹ?±¹YÓ[a¿î³
=Ö$d¿æ@sÝGn?Ϲ¢x`¿é\n•à¿ïÿÿ²}@UNASNone?ízJø&j¥?±_Ò-¦æZ?‡:̛ò?•æmÙþ<#?±FN«k,"?¯ûî.CÁ?îB4ã
ºí?®䣨0?nz.ÁHná?"é9·)u¨?©õã?ÊD?¬Òƒe]|Ç?ìêÚ22è™?šœT¶¸ô,?†å•ðéÏñ?xkÅ?^Ú0?µÌ{°K<?˜ò‹á¤õK?ìqµàVl?¥MÔÛ8¬	?‹siÆÎ ?"Šƒê…Á?¹á²Û?¤6gê'(Ù4FGL J1855.2+0756¿íQ<ï°¹@/«NiÀ9µÕ×7‰ÚÀ:Ž~ŸBP@!ÑÞÚkq@íê‰v5ç?Æ£Þ×fXÏ¿¥Nƒ_ŠBþ?ç§Làƒbö@±ؚ‹\¿ïчF°¾y?ïÿl'ù'(¿è‰î@dô÷¿ëž¾°nÈ¿ãëæŸ‡?Ч÷à÷§UNASNone3FGL J1855.6+0753?¸|(ˆ~Jõ?³Z–£®Ä?ˆ¯Ùe>2/?"ïˆY!œ?썻‰[=Ù?µ.'Íwì?ÔnÑ,‡Ó?Êwï±àÁ…?œeÝ5j ?¯ªÐážs?äå/`Æ?ÊøÀҋ¢ª?Ñÿjy~?«Ý€'ù`¡?µâp-"¨ä?ž&>Í0´È?ä¹²EëÛ?¬î‡§±""?¾¾ïàº^Æ?ªÞ·ÍUŽ?pMùZ¢,–?kòN:–×?ì†3oÏ?«0Ð7D'¼4FGL J1855.2+0456?ïí5š°_?ösC>C1®À8(ܛvékÀ:ð)É'&@\àb€Ô@¦»Ò©†?¿õW°kP?ÉPx‹H@Šu¿Ÿ½ @Ê(K£—t?êœËbi¤¿Ù߀®'¿èº°ÕöA:¿ê¹ËhH¿¿í2Û>Õ}Ë¿ïÿ8$3»ïUNASNone3FGL J1855.4+0454?¬àU¾£?¤þxY;r?Â6\ÓXâg?Àå'T	ú?é±gM$k{?­RÃMy?£ÇFº#yF?¨K~t-?Ò»ªhœÌ?ɂ¦	›,?åe¶`Wú?ÉÙõ€N]?ÁJtÅ÷a¦?£"÷=°?ÍBɋÆ|Á?°£ï¡Òç'?ä\°kˆf?°yèÁŸÑ?v3sÐ?uRtÛ?É©¿Y"4î?ª*Ԓ}[?é!3ÓÞ¤ö?ª±RÈaš4FGL J1855.3-0740?Ƅq¥<nÀgϽBNÀ:$ÀwSôtÀ<…
š¶@#²…£Ã@2ƒZ'ó?Ò͖‹È¿?ﻜÞÈwÓ@5ÿñ?ü€…S'wŒ¿Ó:9LQè*¿ÂùCbÖ9¿ãle¹˜<¢¿îUĝ~U›¿ïùzu$?鉸 šê§UNASNone?³Dv
‹Û?°r\Âïoh?ÃצɣLÁ?¿® '×Ì?衕ÞÕÛT?ÃS45šÙ?°­Õ'uP?·Áò›Ú?Ý\?ƒ?Ïõ'Ü2õ?Þxo[Õ¹(?΀b
ã`™?ÈæjÅ9îy?¥/–¨ý?ܹUrQ?±÷@ðé)?ÖÓu+W··?¯wBs4«?ª
EìÖ?˜ã"ÑE~b?è3³ñ¤I?¶6ÒÑ¥?È­Ìçó²V?²×»'/áq4FGL J1855.6-3603?î[kǵqøÀ0\'IðåÀ:ý6¤û©À<©"¾péw@ð$ÃXÚ¸@	üD~?Ò2µ^ñýß?êb–P@žӕ=ê@-}C¢—?ïÈb¥Æ!?ä̤S0ÿ|¿ØPêh¿;¿éÛÑý¹(Ö¿ïÿi'_Ž¿ïùõ÷h'UNASNone?ÛÏ¿2 p?ÉUþ©vr?à1o#DÆ?ÉÏVUm5ã?®w»6°#?¨ùá+H?ÉQƒñ@‹M?Èu¸¼S?æ%Òóÿ ?Ìüy€Ïû?¼ûɅÞìc?¶Šˆ¶g?ËAã÷Û?­±3×px<?âµ
÷•†P?³pŠCeû?Ééð*—×ä?¨غt¸Ð?³ÈãBÌðº?š8òŽî?êzc}dÅô?­ÙE-îς?¸dÒߢ?¦dÇU·S§4FGL J1855.8+0150¿ë×Fà¡¿ÁvN{c"ºÀ8¢ _ñØÀ9º`Ðû/·@ `7ûÄÜé@ܙ®'O"?Èajh©Œ¬?ÐZãü>T@phÌ›?ýq¤Ýð`¦¿å‡´Nß¿ê#| âΗ¿ÓË ¥<%¿å^ÂÞatº¿äè,ÿèX¿ðUNASNone?̺Köη?Õ{ï4tÊj?œ"‹–›H?©qjšêÈ<?çðX¥_Éy?Õ}62Ÿ?™Nª‰† /?£ÕeҔ,?ª›×z*V¸?´ÁqÊ(Ì?í‹Í4%"?¶©0㙠Š?¸-.S€O?÷ÖÇÞy?ÄrüjvuÌ?¦gûð™× ?çݛòX«?©^¦£?¥"?\:¿œ/Â?Rk5j—f?ƒ
ŠàÎç?yìMŸ3ñ=?塞ÆöL?{ˆi€ðRd4FGL J1856.1-1222¿íg/!´8À‰"š|À9Èé<oÀ;¬‰RúxØ@nýúÂ("@ƒæœ«f?À±ÿ¦™?²Q_>e?ô'|æÛkÌ@5ՏºÉ?é2^ASÝM?ï´6Óѣ̿épÔH±¿Ó'C>™ê¿åÔcšL¿éºžÌßADUNASNone3FGL J1856.1-1217?åeò&Õú-?ÂbÑѾv
?‰Y•j£ä^?ŠbyH|?ÔiOþìƒ?Â0äÈmHŸ?ãChœÆÛ?ɝ–Z%?qž£¼tM?€ü±_dì?Ù2µCÔ¡?Èó$0…R'?äH1xÉ?²=9ŸIÅ[?¡ðÅ¢k¬ª?ˆYE^WTt?ՅWIO˜Ú?°Ñ']Äh?æù2D·JŒ?«‡ì«çY?«ž<½ö?•à&¦¨Õ‡?Í3§½¥S¬?¨ß­ª/Äv4FGL J1856.5+1735?à˜k׏É@R§¢pØ°À9¯0YddÀ;šätªÍ@žç'–òË@ù?ò^VÍ?ËéÖš9?Ïèw"KYp@Åã|;ºÁ?úqòxØÙË¿áZ΂¯rI¿æ¿‹€Ò"w¿åj¤ï81 ¿äªÅ 0!0¿ð?ïýk›Y:UNASNone?κ"r<—I?Á·DÌ£Î?'ê'rŠ¾Ý?â7>'@?çÂ	ç܄7?ÂÀ¨I¿?ØÆL¿
?ÎL0~ñMö?ÁïCþè?Ã)¨K½?ÞXúÌæ?͐ѱ
‰U?ÚÙÀ¦?¯ÀO—ó6Q?¿kƒ‹'ñs? xþ{7?ÝK_
?­PÌ[ŸXä?á*°GZ€?·žkPzN!?²Ý£7E²%? W}~ªƒ?Øó6£ÿÞx?¶´ÅCÔ9ü4FGL J1856.7+0125c¿ï	i‰—ª¿à³PßìdBÀ7–|ÿ/¨À8Ö5¹ö0s@ÀÈGW@u üÏÊ?Ï(ퟀ8u?Ù&݄ªõ@MI€|'"?úCˆ¸Ë¸ü¿åە"d~?ïÈpçɨU¿Ú¬)žßԑ¿çÝÊD\P¿ïãÈ&tÞÏ?èëï<c]UNASNone4?'‰"ð"Ń?£/ŸÊqôý?›Á­kp\?¬r¯}ó´ƒ?î×Ì@âl‡?²<aêþ?–vN­¤Lþ?Ÿi[›"?Î"
&±ç?È/vq½rÙ?çƬ‡I1?Èf"ãøî?®x0µF?'€sý)?ÌYÓÒ×N?©˜ƒÀ(úô?ç(gÿù¸?«\xžŒÅ?@ÎÛþw¸?>S.Hފº?¢ï?¡	"?ŸÔ§Æ?îÌØWï¯É? D4JÇ	4FGL J1857.1+0056¿ï½¾¨'ü°¿ë-4¶ÀñÍÀ8…äÅøÀ:c®ƒ5ª@ ±—è¥@[ àJX?ÁºuÝ&â?Úg§cܞQ@9Úak@Ò¸¯3‰Å¿ïý*,ú4?ﯴޙ}ë?¦tûTŸ"…¿ã«ón!EË¿é-¯›cž5¿ïô‡'YY8UNASNone3FGL J1857.2+0059?Ž~›.?ŽŠ<!S?ããÈ%ÑÕ?ÎIĔfê…?×DsÃÍM}?Î8"óf±ß?‹œDTê¶?•<ñK6úk?Ö|s"È[?É	@mjz?ä"Pµðú?ÈÝ WI¤?¯'='µâá?–£X¯E'?Ù	§~ξ?³î:óÝ£O?á†WYÅ:s?³•E'*¨?ƒô:A®?nk}¬f{‰?Ê°O'Åá_?´‡|/6úJ?é¤Ner?´¹PÚEK4FGL J1857.4+0106¿ïöq+;m¿êmjf¦'GÀ9¶)XüÀ;%ðÁž›a@ ¯®ôŸ¥@—á¸íø?Јñz+??ïÜ`w	L@h½=ã^?ó"ˆñ*Ð
?à'5Œ©Ç¿ìؑ[Ývh¿ÔbI€ýk{¿ÒtDöT0¿ì³L=pMñ¿äëIº^UNASNone?q2ù»I?q؈=£Ï?Ò»Ç.âÕ°?ȸ;'žñR?æ¶ur–?ȼ…I;R?……bà/–?"Ú€¾‰"ª?àCøêÔ?ÑÚÓÂ(	?ÞËãÐâ{?ѕtsݞ?¹×ÝŒµ?ž:­nÊâó?×Ӄ"Õ?³òøZÿè?àÛBÔÿ?²ÂW7SR?GÂ?²¬?BòܸÞZü?èݼïó?Àó;¬Í³ ?ÌtJMŠ?À鯀Ã$4FGL J1857.8-3220¿ã%y™ž÷ýÀ.¹<FØ+¦À:#õ|ï>èÀ<ëD‡Ž@Œé‡îv@†ó{??ÄoÒ Ì=Ü?Î0/ȚŽ@¢"›R×=@¥¦Z?ï'ãt®þ†¿â†?ʛD¿ãø]߯' ¿åóÂ[.пéâ6'¿ðUNASNone?çÅü(óï?¼¯˜Â^$£?¶ë!1&9?­Ÿ¸c^D¼?År~ٗ°×?µ€ˆq+ãF?뙮Ò†?¶Œ¹À`›'?¦š&V¸‡ù?§SÂóq`W?·åvCç‹?±'›K‰E?æó<vzƒ?®"ªƒçq?¶¥ÇÊG¢?ŸBh2ä?ÈàƒÆ@ò#?¦2Ø&§¾?äeáýåØ? Ð±Â(I?·ýñM§¯a?"¨´ˆ¼ï?ÑÍ·èšHw?ž¦ÿ"ŸL4FGL J1858.0+0354?ë Èxp·?Óу€R ·À7òŸûÆÀ9ß:Q4¥ú@*ÜGéùƒ@@öÍ0 ?º¾Ä÷@hÑ?܆—^Uö­@!
hn~bÜ@dªõ°7¿ç¿sFS¡¿¥ÁÍBC‹¿à'" ÔÇ¿ê_@z¿îJ}ғ¶¿ïðÌö%ŒUNASNone3FGL J1857.9+0355?€êTG MË?zëþbηé?Úq•Xv/o?̾ސÿi?⃌¨g?̱òˆ)3P?…cõv²-?ú¸i­1n?â¿;÷hs?ÍT'Ðñ	ˆ?ÙÖhf=²?Í5Écùç?™µ5wMñ?‹#œ/*¤§?ä›Êt€?¶c±37@û?Õ.ªÍ¢!?µÖ¡ñMž?a-J
²æÈ?Q\ÖÊÊ%&?̜ÔBžÏ?´±—J`àâ?èǝ³$¥e?´Æw†²e4FGL J1858.0-1052?ÙD¦HÍÀÙý6÷äÀ9ØB/OxäÀ;U/‰Z‡5@ý¸G"¤@dÐd1@	zg9Êüé?à7½½eQ@Y" ä¶?ôfxÚÝ1?èc]c2¿Øì#"¿ç_¿ž ß¿èÄ® 'Û_¿ê"•%–'~¿ä¤²Çë¼UNASNone?Ë>#ýþ?ÀS¼Tz+	?Í_ž¿ãé?Æ ìÔ߉ž?á؏~Ɇ…?É÷S–Y‡Ä?όT-Dƒv?Ñå1[`u?Å(ñ`û»Ó?Ï	xšgü}?âÒ®œoð-?ÑYj}QÉq?Ëñߘ4?¦jÆÇÖ3i?Å%ˆþ£[ƒ?¦žøÙ"?ãñ!yŸC?­§Däúя?ޔá-]¸?×Çyø.­?§†Y6ÕÚN?Ä.˜"Êaå?ÞzSÖ÷æþ?Öý»":sm4FGL J1858.3-5424¿ín\´sÀ6¹øã¬cÀ:*z¡†ÍåÀ<jñé¼Çœ@µ[ d¹é?ÿyfâ?¾ét£@‰?ڛaðµà!@?ŠÒVy‰@öýÝ;?z!.N¿ŸOZ±&~¿Û9NÀ­YÀ¿çㆢ›öÁ¿éA6ÌD瑿ïó³KUNASNone3FGL J1858.0-5423?Ã1ƒ«|ð?¶Ûeòق?ãô	UWf‰?Ƴ#ûÔÿ
?ÌþVÿ èê?Àú§g¸±?Õý"D7=?Ȩ{x#Ð?ßq°ã{¤?˱ŠÞ,é?Å!•°›T¸?¹ 1åj?ʱgI~…?«¼®oi?ãXKn229?³5ü•:þ
?ț ßí¸—?©ñÑӃâ?ÚåðŒ§£?¯ü2²K€?Óè)sdíÖ?³OæL³?Ñ1åÿóý‡?©/¥ÄG‹4FGL J1858.3-1318¿ïUw©ïÏÀŸU›=À:`þԆÕrÀ;÷ˆy¶¥C@Ä2¸V@ˆÏa҂ï?Îà'&ˆªß?àFƒÂ—¿¥@¯-šlþ0?ó	ú…Õ¯?ïöëN˜ˆ¿Ñ‰¦ÝNû¿äŠ&_Z¿æ,zFíû¿ïÿ®k¸µ¿¿à¿Z=¹UNASNone?ɸÒÁ&ðà?»€‹:x?ÒÈ̜"Ùo?ÄwXDîÔ?à-elW?Æ:¤>
‡?»e‰f'P?¿O‹+›¶ô?Ñ+nòDÁ?Í`ƒ?a9?ä	›Õ°Ú‰?̧Aˆôø4?ѽ¦;gÿç?©£‡æ2äØ?Óä>…u ?±UÈüꎹ?Ú^?Šø?¯ú
-N™?£ãÈ·°?ƒy‹7sã?â-+©µfZ?³ ‹Auy?Ù)H"~=J?²ö™àj0´4FGL J1858.5-4446?ïç–ØM<À3ì«Oœ À:vW&WƒÀ<X£Ò¿ô@²çÑ`x@ó8ÜÀ_×?Ç«µ¥é´?ÐLI'@ÃÏ,ù]O@ˆñ«©g?ïþaßîé¿àv'=\á¿âÑD£ÿ¿çg)ÚÄÝ¿ïüÍ{Hu»¿ïÿÚ@RÖgUNASNone?ïA… ÃÁ?™&h?©ß?›ãçç*?KUDê å?–)ÝWóòø?•B©Ô?†¼?ì³Ô·\a¡?±e76ƒ×?›ƒœ§Ld?¢Å¢l¤?³€–]óá?©Î`Qñ|?éBÖ¿Ûkw?ª­=fÍme?³LRÞûD¬?œ¿%Q¾~±?ÁN{'¯Ë?¡•¢hG¹†?émÒ Pá? ôéÖÑØ?³Ÿ­MXhÆ?˜_ªj?ÀxÞØöˆ?™`?K¯$4FGL J1858.9+3636¿à4ÃJåMï@,Êl¬Ñ…À;l–+PÀ<¡gSÌ/ï@¦å‡ƒÂ@ÀµgU?Ñp˜ïO®"?äý t-Þ@?ý¾Ý ?ü>t.ûì?ìÿ¢AÞÇ¡¿ÍÛF7Fé¿áò?£%¿èñ¡Þ6¬¿ïþ' ¦Ô¿ïÿþˆ0»ŠUNASNone?à7&‰Ú1{?ÄÝ¿ºjh?ÖC÷Ï8BÏ?Æ͑ã+÷?›v:&´v?¹üs@Ó,?Ì謟¾'–?Éê‡úV/
?áhKø6¢?нB!n{?Ω²0`¢ã?ÅèÂ"ˆ?Ñǯ†žâœ?²uìáÄy8?ßw<gݟ?·kSÅN¼?Î1²yòŠ?­Ò•½ïÔ?ÅäŸ}æ÷?¡í[}è?âm"ïol9?³¡V)	?ТGÑb4?¯Pp$¢<4FGL J1859.2-0706¿æن]k…ÀÒiߗª¬À:M5fêåÀ;º©¢%YV@yc%¿,P@c8´|sï?ÓÝÂ=|¸?Ø\ø¾îì@	¦~â^.Š?ýrö6þnÛ¿ãÌÆ폻¿pjwÜÊ4±¿äÙÝ¡‰¿å•;ÁL;¿ä'̘ÊfÁ¿ïÿOÖ×èŠUNASNone?έÅîO"?»®F]ÇÞà?Ã_
<…Ï ?¶¡}ǗÈM?㤑?bøW?ÂK$–jÅ?À3£ÄAO?¶ÀFXêÐ_?¬ ȏ¥_?®nРè1?ê2åf½Ö?º›Ŧ«N?ÖÇ©ë*0ù?­/?°JK?º!,vÜ?¡)¼éOÍ?ßÛE~š`ú?­ü@OgÞÓ?Åþ€¨Q3?£

™Â'á?Å-xµ×?°ö8ÙÕ?å5ÐՋ½?´1…³j>4FGL J1859.3+0058¿ï§é_niY¿ôðT@Éô«À8ƒÅL¥ËÀ:7m´Zæ@ ,½¡W(@N&&v‡?Ć<¶µ^?ÈÍî_ï~Ó@•;Ãûló?ý®àË¿ïÿï~Óo©?ïÿûB«÷¿ásœ¯ÎE¿åm_[°¿ç'sýþž¿ì>†ƒ<`UNASNone3FGL J1859.6+0102?­\ÀÙ´™?®½«±*4u?ºâÕb©?½€ìºX?êÍÙF-¢B?Á'X"¹Q?£($ª˜°J?¤Àá9o†?½Ú')ˆÿ¤?¼¯Â¥wEâ?ë+%U?¾¿­i8?º˜(¦?Ÿþw‹¬Ð?Ãô—›x¸h?©6žðs?·?ç¯×|Ï1?¬°á
(Ê?•é¥B¾üj?Àq÷¯Æ™?±ýˆUŠu†?˜µºò´ã?íË8¹m?›ÔQ
¿JF4FGL J1859.8+1545¿å±ŠÙ"¸ƒ@-ÙÝV‡ÌÀ:²€Þ·°ÜÀ;"''Û\@ •ù&rª@Î!¾–©$?Äk6D_«a¿´à!tK×?ó߄•%–'?ÿ«›úœê¿ï@†}ˆ?ï1KgŸV¿îû"‰µ ?¯•pkwó¿ÓûpcÀCÒ¿ÎÐE藃•UNASNone?À™}A8Þ?¼pÓ[)Õ?€`PzmâQ?…Þäƒ?ë˜mÖ:??½Á7z'?â&gݪ?ËɸUõv¸?"
.Ùߚ¬? á0åBèH?ÛÞÍÜù?Ëî¶!»V?Ù ‰¤‹Ù2?°2°UA3Ê?¥°žŒqâ?f+?wr?áÔ±Dòõ=?¯t¶Ið6?勃Áv?½Õ>Æ*?}\…õ7÷Å?z÷×¾$ÛX?Ôs‡À¨å6?¼æåקÈ4FGL J1900.4-4941?»Û 2áäÀ5½Å?9ѳÀ:öwZªpÀ<‰Ü°ožô@ëzPÔ@üÁr&?Ï8D,ï?×øúRAt@	ޏh"@p¾®üØ-?ïû¼¤`œù¿á§±ŸÊ¶¿ß[Á•â¿âg)¿ìêz¿ïþÕÞn_Ú¿åSu}°"îUNASNone?íù.‹mõm?¢ÉÁŠÑ?"ÿmì†cN?'.TZ2²?¥í`RÝw'?œ²'x-'?ìIZi(R?´Z5ɈFŸ?ž´ÆûΪ?¥'Ëw?¶,J÷ÉÇ?­ãÉQÐè?èJ<Eg´Ï?«w—0ñÚs?¹²9Š§¹? "‰Y³Ë?Áýòi›Øê?¡^Xä?è^e[›r°? ôÙÂeŒ?­â(z³$†?'•ã"õæ?Ç
àrål!?§æª‰ê4FGL J1900.4+0339?ìxï#—g¿ÕÕ° CÂMÀ8'_3l>À9í¦Ý@ø.åƘÖ@¢=ú	F?¼üÛ2k71?Õ,áàZH@IS.Ô)@TöÂ>©^?ïÿý{ÁA¿ÕbàõΤ¿ãCàµ7¿é)Ùîm¿ío¶;ÏÆ¿ïýŸÝÂUNASNone3FGL J1900.8+0337?‰¥B+4ب?'4Ý£6ÏÐ?ޖœâ2¶?ÇvÙ¹Pn'?àN†:&B?ÇtƒN5HN?'ü³õ o?—ò'o×7?×+H«0u?Æ¿q4°ÉŒ?ãå»ýúÃ?ÆÇ'‡Œ ?®q&à
?Š4XwN/Ç?âZ®×d©¾?¹þsy²?Ùo»>È«b?¹$wå
?fEm8Ǐ;?TÍ$&¡÷?Ç
ý²‡0?ªfÐ
ô¹½?ê&û&%lp?ªšB:gI4FGL J1900.7+0426?ïµ5EJý¿§•TÝÊB{À7ù܄д¹À9‰W[0¨>@Û|_÷âO@tåÕ²Nœ?ÄÓ朁«?ÛpÇþ±Ì@@ õC
›Ê@"GÍÉ÷Û¿ïAhë{ä}?ï÷Œ"÷™)¿åœzŠ	ٞ¿ëj;=#¿ïÿöåv¿ïyöуóUNASNone2FGL J1901.1+0427?¡¹ý¡¿?·|RYU?²œ3¨(Ó?¹åáÁúŒ?ì"ty°êª?ÁÙ3ºfZÜ?Œ¨›çÕ?•üÓ\'(?âÿ[	ÕKç?̉
o?Ù '¯ˆô?Ì1ðTħ#?²MíїL?¢ÊUÎc?ÓX9°t—ˆ?´dL†\]{?ä™jS?´8½F€ø?Xbakg"?Iێ1r½Ö?Îäðþk²`?¶øÚ²Ô?è:µ4]´?·)Í´˜y4FGL J1900.9+0538?ÏeÓ¢®?ÞJ}ғ¶À8Kš2EÍÀ:%øÛH'@"ÞÏ®©@¤A"HG?ÈÞ½?ÚW<'W…ù@%B¯§ù@å3éf‹z?êàŒ1Ò
#¿à«µ?èM\¿è"³!*¿é"Ýr6~A¿îØú!ï"÷¿ïö[ ¸lUNASNone?€aM<ìè³?~8wÓ&Çe?³òpÛŸ?·" 4}dò?í@8Üðé
?¸&´þí?•
ö,÷L?•¾ŒØæÞ?ÂӌG>ÍÁ?¹¬ÕãžÆ?Ꟗ~äÕ?¹÷™ÊÂr©?±@9"#¶?''¢'k?ÇÔ$~†ò?ªpH"¿š{?çâルþå?­O8Ð̂œ?p
6]C?Ò?Z¼›¾ÎÓ?ÇîÝ͕žÖ?¦`J¬kRØ?éä4àË?¦–Ž=ÔÛ4FGL J1901.1+0730¿ïÂí8ZÂø?ô9ÎÃG
À8Éw'ÕÀ:vnWÌp@J"á+~‰@%4åºÚ\?½ûÔ¢.=«?ÊBIP«éþ@©Ô#Ù?ø€''Þ@?ï¦~^Õ£`¿è¹Œ~($¿ãá"=‰ù>¿ä˜Õ^–¹?¿êœýýt¿ïb¾‰¬½UNASNone3FGL J1901.1+0728?—N[½"ƒ+?'ø!U?%?ÁñÉ8ç?»GmnÕ©?êÉÔb ?½2JÇ._³?šÝ}dŠ'?¡õOq­?µâ«Wñ7?µ3@"Ft?ìˆw¿p°ô?·ÐFð›•?¾h\G¤…?ŸI¢Æà7?Ǖ†¿7Ñ?©¦B!ü?æM'Ö¬Ý{?­%°3Í,?~ýh"úǑ?lè"è˒?µ±•k'É? Ò c/ªT?íҁ}¸7?¡¼ô¤BØè4FGL J1901.2-7307?é
A©eÀ:"ŠT'À:Í*ô PmÀ<>é<o@FìËï?@7?Ŏ")uš¿¡¡ÛÇ*?Ü
ý¤[¢@F‹OSû*?ïù–Ys8Ý¿ë6¹ÀU›¿â¶ïö1J¿æ{þ¤Êû¿èíݾŒ˜¿ïÿ®XëTUNASNone?ïŽ]uíØ9?‰ø{ÔÏ?WBv"lØå?Q|gÌ:kd?‰€S³üV ?ˆ¢®0n?ï?¶ \?"Eh¨Hâ?R7V$‹$?cZ/…%½›?–嶒6j?'2òí/6)?íÐÖØùS*?•m[0Ã\E?{í4Tø?m-Œ£¯êc?¯tëåÚ¬¢?"ä'–؉?î´É1Ä»?ƒßMôTk
?icö·¶?Xó'kŽÃ?£-†"˜É?ƒ4O>=4FGL J1901.5-2208?¹Pìiþ©òÀ([åÙäÀ:ä%hoUÀ<G‰ßrï@§Z
ã@u¦uJ/?Óãĵüý?×-KþSý@Ae%?ÿôæ³]¿ï—Jy Ö?ïüŃ,oË?œ0G¤í¿åß~ØÕ¿ã®ÈáÉ¿ïÿý¡UûŠUNASNone?ìžÔšaú¥?µ	a ª²œ? Ð™"¦Œ?|°WRuÂÙ?¸ÕAËÖ
?´iG•ÿ?ìF֑V"?¹‹ÑæRh?"ó󶘐V?™?÷2¯Q?¸ÌN‡¥»Æ?·Ì	µ:I¡?èj»jò:\?ª§ïàéZâ?¯Ó€õ9QÏ?–%йó£p?Æ`2èÂ?¥ë"ŽK?æžLÖÑö½?©mxÜän?«yBHV?˜µëäA@Ý?ξîT&$s?¨âúœ‹~4FGL J1901.5-1112?Þ@î˜àJÀ;õ4v)À9ÇgŽ"'¡À;g2:å¯@Á"°Soi@"Ê<ϔ'?ŎºÈ"W?¿ÇñEÒó?ö®ÀWs"\@éz"¿ïh@[9â?ï{Ø»¿åæ8¨²f¿ìB­Yiþ¡¿Õaà89'¿ïù»þHoÛUNASNone?Ýò1¼ç4?ÅlØ\©-?‹­Ï=ׅ ?‰xpšA…&?à˜/ä•á?Å%ËWˆ?åˆ'4hñ?Ȟ™YT?s ˜sÕŠ?'ð۔–™?Ô¡GOÇÚ?Èx}aԋ?Û1'2 ð?°@|'M˜?±µ…©'?"~mþ?à0›
êÖ?¯c'®¦|?èó&?«½w´0?"÷Y"Ö¡€?‡sì^ðz?Í,ع¸"|?«=§°4FGL J1901.8-0718¿èÈ\ù̓À}ŠÚ¹õZÀ:h'Β À<ª/@Kˆ{º
¨@$~d‰í?ËO¡¨Ü­•?ÜâÑ[|Óe@
&‹ýϤ@Áeý4ô~¿ïþ'A¶ƒµ?ïíjWŒ¯¿Ú
7`"j[¿âk8þNO¿ìÜʵ›X¿ïýÍáéOUNASNone?ÆoÏtøÍ?µ´í}$o?ÓÛÐ& ?Á˺Òô>?àvˆS϶=?ÂvÜ«`C?Ȉéò•ç?¿M¶|~"?¶Û۔ñã
?¶ÞÒ¤Õè?ç"bRå%?Â̋Ùp?ÖYƒ0i@²?°;1~É9?ÒÈd–[£?°}µ YD?׌´kc«?®k§  r?ÜPøèó®?ªSév‹…?Ì
÷eÆäç?§FÆ[1&½?Õø³T3™à?©‡YìÙ>4FGL J1902.2+0448?çv/Äé©|¿Ë'^;õy"À8	Î^DIÀ9¥ÙUqK@+d²Lö@ãU9î8W?ÂJüèôJÀ?Ö–ä¦è@À7OøeØ@GNs*š?ïìPU'éT¿ã†áa¯H¿âÅîAÁn¿êX/ž‹q¿í]V½{öñ¿ïÿ§µ¼UNASNone?"kÄ5ù ?¯SÔB9?²zè^ÅÅb?³è'"'È‹?í`AEoo?¸þu¥+‰?•ˆ!:°s€?½­p©K?Ñ8=žÄMü?Å«Â:¤ú¸?æ· &ÈUe?Å°\×êÀ?¡çŸõò)?Šô耑Û?ؖ2æÌZ?¸}Õµý?â–l¡*°?¸ÂPº+?RzP»P?DØ2lX?À†RÆQµÚ?§ÂTW4ˆ?ëÕdC4ü?§ã¢ò߀4FGL J1902.4-3417¿êÝ9#"éÀ0üÑc4'¿À;³*dW˜À< îؐ@¼´B½>å@elÖÂïÔ?ÐÙ¬SœŠ?ޔ¹ËhH¿@½í@?ü'Ð4`YÝ?ïÿÇ`|Aš¿Ûò¯àWîÿ¿ã³ú8?ân¿æ-ô/¿ïÿ‡4<G¯¿î^€SwvYUNASNone?ëáÏæ¯&?µú•™ãµ"?¤«žqÕ?¢Ê<փ¡?¶›ó@7–b?±=ÔC¹À?ä€Ó·?Íã!['ëÃ?Ê¿€¡Êr?Ƀò\š?Ãëô\ñ?¾jóLâ?å'ãÞ±B?°áhëÒX?°ĂHã6?¥¤ìHÿ½?ȯ¬ò×Å?§܇¾»?Ò<Ȑ¢?§½(XC?Õn¤ï6ò<?³¾žu6øw?؍VÔ}!?³·ùn	\4FGL J1902.5+0654¿ì1:ᎌ?åãÆxõµ#À8ߜ‡Š£]À:q=V¢¤@þ½QYº@#Ï!?À¦cAøD?ÎBðj‹º@x¼œÓà½@-ÙçÁ¿îܼßCòÉ?îÞgߍCË¿Þns恩¹¿ãª?K¿êŒ?ÿIvÁ¿îìÎÊÔUNASNone3FGL J1902.6+0655?£…­KÇ)B?—G¶€ó¹,?Ð%×o¶˜¸?Ä>>¼Íh<?æ´¹shA?ÄðRƒ"ë?§B¿¦½´¿?¦kx²"sº?¿t9fË
?¾x·"|Kä?êLØЋR?À÷Çий?À5ÞE‡q6?¢dÁÕô ?Ê {ÅÅý?ª4…wv	?åRÀO¬²3?®(H>é?¨Í½{ÐY¬?"w=6_œB?³Ò&IÂú? V£Yœ¤«?ëøßh9Â?¥ýU
ëÀ|4FGL J1902.7-3246¿ãMž]<‹À0}»úëÄÀ:ÀÉÓIÀ<'oF	@dOÞ¾Š@ZR[íf ?à ð¥ïé2?Õ|8V1?øÞ<Pé'@^¬èÖC?ïü"ßphs¿ßÆí$ÒÈ¿è·ù1~'¿íÀ^à
AL¿¸¹÷2ú¿´¨¾û}å3UNASNone?ìîyÙTq?¹på?âm;?¢î¤
?µªÁŸð`?®ýtTËä?ªÑuë¼f?ìâÉʏ§³?¹ýãªd½?™V<¡ýì?§£X}­êp?²¨\ZBí?³ÐoVÊßÄ?èáR@´*d?§ì/^§Çf?­Þ"=犾?–Ð4ý_M?ÅíµsÁ?£7§í;uù?èÚ8f(F?²J;Tȁ?…/'[¡ç?†ûÜ_4P?ËD-0¶¤Ç?²s(8lÓY4FGL J1903.5-0825¿²—èƒPpËÀüEßÞ!‰À:½……`ýÀ;!| dŽö@µIX8¦:@/ÂÝ_Â@zU_­å?ïÿûB«÷@
?h£Wˆ}?ý[îQ"ñ¿áô€oüè¿çF©½S2,¿ã‡Í¿;Ò¿î3Ÿ¿£n…¿ï¼ú\Rn¿ïif*×DUNASNone		?©«¼'g|Q?¯ß{e…®5?ƒd܎lUV? u^º¡1?î°Ä¯Öå?²LTOSò"?Ò¹pîcw?Ѧ˜¯µ_y?´3½¡Ò¤€?ÅHْz]?äÐ
Îy´?с:/KÊ?ÒÓÒGéûÃ?ª´Ù¹_?Âã.ðÒ è?¢F•~E?áÝKÖYä?¬0MñJjæ?áŸk6Nq?Ù+Eí4›?ƒ÷`"ë@7?±¹žãG³Ñ?Ü!nŽ8	?ÙGOŠš4FGL J1904.0-5925¿çCf×ý"À8­f8C=lÀ:÷ªëÑtÒÀ<ibXº¬9@¸=Qo@ò
ú/§?Ðmn-E	?ÖüadôÌE@ð#̍ã@°StÇ'?ïû¯8gOš¿ÞEý$ÙSC¿â âiD¿éíŽ
t¿ïÿçáüú¿å¨<b5ÕUNASNone?íÎMœÒ?§!¦ŠdÃ?…YŸ—åÏ?"Ç¥T*:?­ÄâQ	q?¥‹	È9Ë?ê8U¡Îì?¾ûmÈÙår?­ÚÌÒQdð?±úÒq˜a˜?¿OìˆfV*?µH	a"~€?è]&Üß$ ?ªÞSý]–—?µL|–?š'-ûž?Ãå$Îxè5?£ú*þÿ†B?ãñ¶ÎÖ?¨‡Ã.ªï?µÕר[òw?œëà,Bú°?Ôr¦¨Kÿµ?§b®¨I4FGL J1904.6-2713¿ï¼äMê;À-tG䛬À:
Gĺ¯"À;ãW4š@×K±Ú-3@±eÆ-v[?ÅuNá|Š?¹"{?òÎ|Iýz@¨_iX^¿ÕýŽá"¿Ã¿æ<æp–¿è—Ý6§[ú¿ãÿšr¦ç¿ïY=SG¥±¿ïËBôqV"UNASNone1FGL J1904.4-2725?îŒÉ«Í?§ôõޛ­a?''^½ï8ƒ?"|¯Ï;h?ªý[¿)u?¤"ª·ôS?îèͨó…ø?¡ZD«/®?k·](°?{엺§%¤?Ÿo_<ŒÝÌ? @nŸk ?êu'sÙs'?©òîöÔ? ëŌÛp?'"-ù\?Áð¿6ü‡?¦&ç¼ä
?ì`ù`N¦?œŸKds`?ŒÍL)iÏa?uVKF₰?¹^‹z¨Pã?›&Aâ¢í4FGL J1904.7+0615¿å"€è?;w¿·íêÿ'ÇÃÀ8ãöíôÀ9úio/bÄ@*VgjÈK@¶ÒàD²?ӕ`˼?áDpù…@¥Y³Ð|…@º>èÉ¿ë*: bK$¿o*8sö6¿æÉäð°ä¿í­Ôï°ýc¿íÛo'C狿¿¸à[ÊÖþUNASNone
?z¸Z/Ü.?"Pٝ‡u?Šø"³¾c¬?š#E¿LÚ?ï^¬øÑN?àÆ´­]?¦…[ËPÂô?¦µØ'õØ?´ÿÔkûÌ+?´Álm[ü8?ë÷¯µËzL?·¶Èš‡"m?µ@Ú8³ç?"ô—2Ð?Ä"څڧ?£€gL0›+?èO.rõ£?§-šÅ€h¸?€Òșþ?p{Lþ("ž?§ðFx%Ïð?"W†	q?î=°vtÉ?–*T¼×"14FGL J1904.7-0708¿ïTꄇ}|À͔ÐÜüÆÀ9	wx¢À;'j¢5IŽ@)­RÞõ@3=??´ùÖ_—ý?×Òå XO¢@­H÷Q@xÀƒhTÓ?Ø÷}šµxr¿Ê!¯'Jq¾¿âHV°æ½9¿è6úh‹¿ë=¡ìNrT¿ïÿí )k3UNASNone3FGL J1904.7-0708?©ãLcžM? À¢™éN?ä\P1ÏÅl?ď@˜´"?Ô
ïrÔ^?‹æ˜eX[?¦t®cÐ>?­Æ…Ø"FÞ?ã0½ÃÑ=?Ë::ã²?ÖÏî«ã"{?ÉëÇ´c²?½0¯þ¶Û?§5œvоÅ?åñ^›"9?²¿~¹åÜ}?É¢.ðO«?«Kkóފ?´å#ü?'¹*"£[j?Ý«ÀÇR´u?¯¯‹¦ßhE?Ýø¯¼‡Ü?­6ƒ\ 4FGL J1905.2-5120?ïú™ŒŒŽÀ6ï6ÍòfºÀ:E£_9MÀ;ø(/Éò'@4êv*ÿˆ@-ô!¥l6?Èg$|a$ˆ?Ìj¹ºv^@ä ¦hµ@ÿ¬ãÎF¿½¶˜>6Ö¿âL¥)ð"R¿æR¿ >yb¿æü`£®ÆR¿é›r·­¿æ£Á`]öUNASNone?ê%ॵ¥J?¶Þcrb
?¨œ×«Roƒ? ¼nÌʺÞ?ÁAG~TÎú?³g"#&?í4ÒÅËÉ?°8ÖÖ/?'LPfë‡?˜8S¹»&?²[ƒwæ×?ª'yI?°?èšì€Ù×?«A˜9bÿ»?¨_~§m=?'©Tïç?Ç|n ½T?§*^°I¬|?çáƒ-ofX?£@ŠÑœ"#?£ozaT?ŠMšG"­y?˞Å*É?£íº†ã4FGL J1905.8+4942?¥ÖËÈ"À‹@2'0aǛ5À:õuD× À<Àêù¾:@à¼z-Ä@»|Bp½Ø?Î\^¥§ÄÖ?é§)¥÷ß@-9–ú'è@÷bõÑ¿à±`ôâk?µ¾ñlê9¿âi`Á¶Ä¿îª5]¯Þ¿É
ý«è¿Ô®)s–БUNASNone?訜ÙË?ÁôŠöõ?ºBê=þL?·ƒŸ÷"?ÂÜ<|'°?¹Ø2p+?ê{p=2J?ÇáÂ52ò?´
§@#?»ìƒFÁî™?¸ÖÕîb°?²ªäSø?æ:ƒQ#eL?²9¤7?ÅÆK¦à˜?®Í­³¯Aà?ÁO§'ÒÇ?¡·ú{ò?í!É!-? ÑBØ÷'? –G†¬=?–×1.ç–[?­M&gÎ0ì?•ô¹">4FGL J1906.0-1718?ïÐøƒcøÀ%æFÞ	À:ÙÒÛچÊÀ<Yíð3c@
æ®bœ@#5Y~ —?Ò߂\L(?ã›bý%Z-@x~a.ï@mMÅ×U?ïŒ3Ÿ¿£o?"2ޛù' ¿¼ÄfKäZ¿äô>‹$¿ïþ
A¢a¿¿ïcoqY	UNASNone?âÌÒtNø
?Ån;øH6:?¶"˜åK?±HTÆð?ÔÅ3±(½#?Äu©aCÙ?ז¯ä·Ÿm?Ì
à²S?¿[lÌ;]?¿4Hôl.ã?àI:tħ?Í»õC…&?áe)`Àßý?±—\¤ßè?ÈkƉv™Í?©G0á6¬?ÐÿÉùÂó?ª:!œË¢·?á|¼?®QxZUx\?ǙUŠÅì¬?­ƚCr'?Ñ;3-$ϧ?ªN•2ä×4FGL J1906.1+1651?éxwHZ.@͉âlqBÀ:¦"Cƒ…À<x­"šB@ Gq=ÚÖü?þ¦öyn€ç?ÏjÜs­?ïmi?^º @\¾Fø@

 •L?ê}K…:¿î›éÕò|?åxUFƒr¿Ò&Æ0<‰¿ì³Éá`È¿ïÿÚ €UNASNone?³"Ã	ß?±ÓçPI‡?äD+xe–d?Çås©³M?Òµà^r[r?Æ =JÙÅ+?ªG°H¾¿?µkzCØÈ?âcuê€Ì­?Ўlþ¶eË?×ð!æ£N?ÎU…X
€S?ÉÊØgzå†?­æŽµdêß?â‡)K¡R?µqc¸ä°;?̃;V•0?¬Ô:ELð?³Ïù¹4bª?¥³ÒŸ´N"?ç4꧃ó?À³H;G£Š?ÉGÓxǾá?º);ÀÏOó4FGL J1906.4-2001¿æ¬»"ûÒÊÀ(VÑ|^ö0À:e-Ž¯À;»üߺ[@隆~‰É@D[Ëر?×µ?¿ˆ—?ãuf´iÿx@`†R•@ðÒæl?è9€õ]县ãE;©#zY¿à†Êßâ©-¿éoÿ¢.â¿íÈ1\™¿ïà'¢ sUNASNone?Óòéŝ²V?ÃÄD.xžë?²–Tû†LÔ?®:¦_¼¶!?ã³À}À];?ÅC>6áW?å8s¯'Õô?É$¼K3§?¶H²´-²¬?¶óæô|ž¥?Ïù×éIÎÝ?ÅèÝŸ;Í?Ün'O× L?¯|0¡?Åä,ÝÝü?¢ÿô>·ø<?؟X¢¹p¶?­u"½óÁ&?ԑ>;gw?°ìšÎʐÃ?°¾µe@×?¡áÄó?㟞ËÍ$*?³=Á*ÆÌ}4FGL J1906.4-1757?ìïî¡¢–\À&™
þ`ÏÀ:_¦FPFiÀ<dÍ	2¯@MÐù^$@'ùºk¡9?ÈJŸ¶i3?Ô"Ãäƾ–@†ý<× ä?ûRŠ.A²?ïôÕ?/c¿àÞ1yÏϿܗ|=¾&—¿áDêÜ0¿íÖé¡éÜ¿ïÿÞ§À£ÊUNASNone?Óóç¤P®?лNåhã?¸ç_×?°º¾?,Yé?ãyÉ)Lk®?ś.…#J?Ù{˜'œ?ËöîïO2{?·‡nϸy˜?¸ÊáÆë?àŒTYú¨?Ífrá>5?ÝdûÂá½?³Be= £+?È2ÚðÍç?¨+Â깉'?ցüЄ·O?°ÆFv®Ñ'?ÙD¦
3Wá?©½
Ø"?ÄAQd?£½çH"Ïå?ܚÓʘ×?­¤$iƒ×4FGL J1906.9+0712¿î¼ÖÒ+©¿ÂöÈHٍ¥À7Ÿž;¿É¯À9Š*^x[[@ }øäWØÚ@˲5qÑÔ?µ®úS?ÉÙ×¢=×ý@A#=ó?õ· ¾œZ?í)#øÁG¿í*ÃQ#?Ùjä$'@¿ãýl§É¿êŒ<ït—'¿ì*úIݙ¤UNASNone?zùÍôÀ¹?´½ÏìÌ?ÉéŸ&dÎV?Ê e =L?éO¤š}K/?ÊvÄ]™	V?}UEdû³?‰LމdçÃ?ÒÛ(¾_¦?Ì«¿*"ª?æ¸çà¢5?̐#Ã?ªVˆdéb?—R¨J+0ÿ?՟iºšøô?¶/3wŸ]Ð?ãŠâœcí]?µ©½ÙíY?+v•?!È<ZÜc?Âwԉ––?¸é'CÆ`?ë`Šcqxò?¸ô¯â¡•4FGL J1907.0+3556¿ÝÞŠ¹Nb@)A?À	oëÀ:؝@îÙÀ<^'ø»@Ò¨'Y.E@žº»RQ?ÐA°dmF?օ/IŒ;@$zü ¯?ÿ[Ô½0¿ïy‹Y?ïó}ü…!¿ä¶ùáØ͌¿è©H>]¿Ü2-d<?¡¿ïÿÿ" 5•UNASNone?ë1ìÐ3˜?´ï[iEù?—i¦<Í_ô?•âÀ» ¸ì?ÀK÷šQ¦?³I¡±Ä›ª?è"¶´¸‰?ÝvHÝã7?®Ú8ž™4,?±qƒ*.V?Åýný†ÐÍ?ÀÒ&Z¯F4?è™ãœ'™Ê?ª Ÿ¡z¥?±·ÇiC=J?—ÕĶ¾—?ļÙú3?¤·ÀîG
Ø?筑}P#‰?¥ëp â¦š?°&ÏK}$3?+Ñõ¥Øâ?É6ReßÃ?¤
·.·CJ4FGL J1907.7-4037?¿ÃCÙk
7À4.gù
wÀ:€ž<–‰DÀ<*&i U
@šã	û'@,ý>" 
?ȵ&gó¯:?ÁŽŒ	äw?ñM¿¦sœ°@¤êÕeM¿ÜÌ~VG4¿Ã¬Ö!à$˜¿èìXþÉÊ¿æ­´©^3¿ïùà#kÀ?ïªóɐØ*UNASNone?î}Þ³¦"ã?ž'ïÜ6c?€õ8â?Š?|Íð"×Ò7?£äƍ
ïL?›£ÇÅ÷nÓ?î†ÉãÁž½?£±}>.í?xSuž‡?†œÿƒ*Ò?¤ˆýÕ2QU? µ`Gúc	?ìziÉ^? «íæ"ò(?˜Ê(än§é?†Ø?2ז?¹9¢x›s?›‰€O+q?íš22oȦ?—+eïƒi®?‡¹2ø"‰?uï&R?°7H
oHÃ?"õª"àžà4FGL J1908.7+0812¿ÊôÀÇ/ÿÍ¿³÷
þp]áÀ8ì8¢Þ½À:™8JÊ)@'Sæ/@'D¦">?Àé+}1Y?ÙmucÚE@VºI<‰ô?ÿP­µ"¿£Ñte6¿çUá"oA¿äÕZXTU¿êޚú—
¿ìtVÿk/¤¿ïþ=RpæUNASNone?{¼
ò¤¨b?5Ò븥µ?ãÇ`ãø¢h?ËI_îýÕx?ØND(‹?Ë*ãzµ­_?"s!y³
?M¸Hâ‹?ÜG69Œà?Êû•ž¼T¡?ኘxyRÅ?ÊçXfíù?¤_x-œ?	±B2c?ÛúñtL¢?¹Îaû u7?༕nXÚU?¹jûI>¨i?P!—{o5?>IGwyܽ?ÕGfH«`?²™Í{pB?åwËŏì˜?²–û!4FGL J1908.8-0131¿á./èZ;ÀHðÄXŠÀ9,­m‹ô•À; mµ@æ@(¬ò'Ø?ÿè˜n#Ê?»KVët-?ÝÑÖÓ°@ ¸Óñ"<?ýÍBŸ¿á9|žCU¿ Î˜ÃŸ–M¿Úié=EÛ¬¿âÑeéŠs¿ï(¦G'þ¿ïþ#A"µUNASNone3FGL J1908.8-0130?'¨"уýÉ?zéXœ£ÏÞ?ëñ! ²¦?¶¼åÞûϵ?¾!ïœÉë?µÒ¾Ïgùâ?y$_X!?•£[5Hžê?ææ窹Æ?ƒS¦c$?Ñ*ždšîp?ÅüÙ¨¿lg?•ÔICån?VÈdβ?ë¯
w7m¶?¢ØêÃç¶?½š3˜ø? ™¤+ßiV?—€¬î°í?z"Ùœ6ÓÏ?äv¥ðF˜?²ôpæ?}½?՚©]ƇÁ?²}ÖÎÿ݉4FGL J1909.2+4646¿àƒ?íx5h@0.3ðÀ;7hWØ.*À<Ö{@›å،s–@UŽäÒ?ÍÉ4¼Ë!ý?ÙT%ò{@¼éåâGˆ@?UÑ{¿Ì?	U>K¿á͊,>Ll¿Õó"\¿áæ—䍳²¿ïìRnaÝk¿ïþß06)UNASNone?èæ
+cn¤?¼Âè½?Â4×ESÝ?¶"ÕhòËL?´eèåã1?¬!›–_¶E?毅Ȭ?ÃØ##׸?ÀS‡çfÁ?ºì	©mž—?Ç9º]èÍ?»y-L¥°(?å`´_ä™f?°6âûw'?Äã—ÚN¡V?¨|ÄƑÃ6?ř–¦ù
?£ˆ{'2§?å˜Y9?ªmÅZF.Æ?Âkâ<½>ø?¤"ˆ3ÛÏ?ÉS©Àá\#?¦HHUç4FGL J1910.1-4704¿©êß$é†À6ŠZ%"À:r·ÔCéÀ<F·`Sý®@8h§3`@J4CÔk'?Óà]7é{Y?åH-€Á±f@eöº «?öÔkçÛ¿èžç·4¿áw—±b
;¿æ¨¿aÕ2¿îì<fd¿ð?ðUNASNone?ëD`aãew?Á‹•ôïU?uۚ}°P?…ÉŒž·?Â?¡¤"éS?Àו~ðþ™?慉…<\-?ÉçÈ¡ù¾Á?†œNã«?ÄW¨½QH?Ãc=œ+ƒ¢?»ÞâÂô?ånÖ@Ý?®1ƒÜnC?ºòø‡?œW1VU$r?Í;.á
F?©·Ö–¥ss?ãDx‰?ºÿ™À[ÍC?»4·4Àm?¬ÿUJ±¾?ÒüIÞìq?·!ÛäRàV4FGL J1910.2+0904c?åQ
ìíÿw?5ïò<4üÀ8Dß-!¡À9òŽù,§(@!;êH³£@PwDŽ¥?ÀZyɹå?£¯a#}Õæ?ô0ÓÊ?ú$ÉâοïšG©â¼ù?ïÿd™ÝŒ8¿åµ)ã(Xå¿Ø•ýB`wº¿ëH¸ ÅÝſаh¾‡úUNASNone$?¡‰×50ά?¬Ðrè
Æ?µ.mu½ày?»¿éSPē?ìA"Ýõ7?À*ZòbµP?¡"°+Rã?£Ë±;÷í?ÀÖ4]ÝWÓ?Ä/Ñ÷ÎE`?ê¸GåÓ{Ú?ÄWü˜¹ô`?»/5=Iù? ';,'Ò"?ÀÀ§«ds?¤o_YÜQ?è–.Ïm}¤?¨níJ¥b…?™Ø"ª¾?†óE º?±ìc¥ÐÁs?¡·‹uÑ,-?ìó²wH'á?£|-´N‰4FGL J1910.7-5320¿Õwoå¸xyÀ8>A_EàµÀ:~ùc<À<b
@@M…XÄè'@$$D'æÐ?Å6w
x~í?ُã¢Ò'€@•›Þwì?øöûú·Á£¿è›n»Ÿ}ß¿Å£œQÚ¾¿ä6žÂÎFJ¿çGú D®†¿îÒWPHí°?Ҕ«]¼HÆUNASNone3FGL J1911.1-5318?̌«ú"?½é&'‹w?á·Ñé}L?ÆÕ}S±d?̗5·<??¿ÍóÄ ô?Øڟ˜úÑû?Ì–‡Á|?Ü?…±u?ξˆZ7ØÛ?ÆFA¨7 ?»+ëO}?×cü&l"?²³±ÞÂ'?×e5´sU?³ã?aZ-?чž¤< ˆ?¬â5 ?Éjƒ}3ì?©?œSD»?á%bã·î?ºÀŒTÂ1I?ÐÿúžÉ/?¸j#žôÐ4FGL J1910.8+6300?ì^œ‹;ˆ@5Ø6¸ù±1À;eszK¹À<åyéÐé'@ .e2§?ÿ`UÆ2o?ÌC">™BÝ?ö©à8º\?ôˆ²ÁˆÌ@{2ü+µ?í‰?MóÔ¿ï韛†&?ïÄ÷u³¿åÎéõÒ¿ÖÍY$3ü¿ïÿÕ7ÕYcUNASNone?ïe
ƒÅjé?"qb&@rÿ?VÆÏi@Gç?U'WˆPlÅ?'ñ␾ž\?"Öt½µµ?ïD8UöK'?™—aô_ã?Z­øÔJÃ?q1¿¢/"ˆ?•Î³õf\?—Á!?Hdq?휝ÄsÊ?£ÒæÉÍÿ?rœCôB?hè¿Ãµg©?¶ÁVØý'?£§Êνáú?ïPÆÛV2»?"9_WÅ?[Œ-Éi?]˜"Úyù?"6+Ò]
?ƒm6xÐ^C4FGL J1911.1-3221?ÛS΃ÜÀ1ùÊâ°À:À1"öÂjÀ<BWڎV@í§¸Á'@Ñ>Eþ?ÑZ¨VÌ?Ԁo|Ä>@H÷}z"@ÙÙ7"@ê?é÷•ÞN)"?ãâ`b@fø¿àî`/뀿áñĞ*"¿îŸg~¿M³¿ïý"€U$öUNASNone?ëpÀß6é‡?°k'g?¢î¹ÚV_?›FA"e|Ã?»œ="?«ù÷Ø6ΐ?î(‹T¥n?¥–Óò!—?"6ì£ÐT?‹ªåˆà?¨u<ú€*?¢ŒÉò1Ê?éH}ê­ô?¨*¼i¸?´m®Ñ;ar?›	ªL–n3?À§4+·—y? ìNԌ||?êZòùÐã-? Jçu׈?¦	C³Eµ3?ÿšÈ¯e?Áã+ëý?›vñ<­Â4FGL J1911.3+1055?ã#P°­Ãƒ?ãgpQ¡³À99ˆ{¯¤À:•¦†è½@¡'Œ_t@íŒ_õ3?ÚBj?ÒËÊCZ°@r=äg?ú=k€3í¿ïõ¥¾Àðv?ïÿŽñ ¿çHÌAâx†¿çË,^WÏ¿í8="ßEu¿ïüÙçUNASNone?ÖÁðäÑS¤?ÅX)Åw,O?Ù]yT Ӂ?ÊqxAz?ÏÁ+Ž±´?Å1õƒSf¤? ÷¹ÙRü©?¦!‹J·¾d?ϓ–Û¹ò€?Èo¾¥µ‡@?çž«|S–?È¡è~-Bk?Àq㆛Òò?œ?¡ dÐs?ʛ˜®'?«Ñv^öFÞ?å<ÃøXŸ¹?­»‡ýk•W? v÷€†-´?‡¿´‰#?ÆõÉã÷sf?º-¼8ëñ?é;ùÀK?º!š'ƒ;4FGL J1911.4-4856¿íÄ\¯i ¿À7B«%(®À;5Ÿ>HÀÀ<óK¯Ri@vǕ«Mv?ÿ-gwžZ?Ðþ!ÃõÝ?èIè^9q@àýÜ9Q@ÊÇU> Ð?™cÿÙ¿y}? N>§?ÄHôe˜
M¿åÂ2᱿ïÿ;2G?߉ˆ>þB'UNASNone?ÙzªÂ[­2?ƚÄÛ=¾?á8©´ø?ÈjšÀ0Ì?±³­"£~?°ÛYC˜ÖC?àsz"?Ëk=jë }?ÔÃ@Ž¼œ?˧u¹å½X?Æ%,Ýz?»¦×'ʵ?Ó#$ÐÜ?¶¼+ŠaÄ®?àp¸4Gï?¹Mú¾üì?Ç>Ù£#>?§K3.I"(?áªÑv1õH?·Ó˜ª­—¯?ÔqìäoÞ?¹gGÂ
 Ñ?Àpà_-K'?¥Â'¬b8)4FGL J1911.8+1447¿Ò[ôÀå@•@?ºÆà$À:-±4ÀÑíÀ;{miç@!A×0}÷'@˜¤§Ö?Âå9?¼®r¿—}4E?ÔïäÿÉy[@æÊ6Åcø?äE~Åý0¿á®å%‰&…¿çÅàŸgŽÚ¿è–•Ù¹¿¥¢¿76¿â›`^©UNASNone?Äû™C¼?º
sµ<M?~E.w{?ƒ<Ü.W²?ꄏ ³î?ºÈB	4h†?Ñ¥/
ýªÕ?ÇhB8¿ÿ?OŠw±ã?¢d¢ˆÕÂ?æ¸*|WKÍ?ǝs·Aí"?×Vwe£?°oˆÀ7Ö?ª
ˆ¦)q?"îæ*ì?âÖÂËç?°'É—-?×üfp‹ò?³‹"Œêã?~K.†"t?z /ûæ÷?ä9ëo»u?³×ÒReiS4FGL J1912.0+0927?î°7ÒnC¿Ìæ'Ú]"À8ÓbÀ:ÉîËû@Ÿ¼wjÏ@£ß¾AÏ?Ëṳ́ÞÇ ?Ô~ÊuÚw°@DG!ý€Ê?õiҩۆ#?ÑώH,¿|¿æ…¦2.Pu¿â¿-§Ù¿æÛWãä¿ïi§Šóä¿éb`¢­ŸUNASNone?ŽC'C$?'Ò' ¸ç?¯ÐMó?¯ÙrË"C?튍.À™?±šàæ\b?šÑd4?ŸÍ±…ý‡¸?¾\ä܃ŒB?º®JJP?ë]ØDGn?º3%M?°®íj¶!†?{?HCŸ¿?ËTv¹ÅÝ??¯5÷ê{Ž?ç¤7Ä?¯ÎåýÄ~?aq	¿)%?Q¥»ñ'?¸¸°N¾,¸?¢³Ðl¤}?ì×xìh«??¢ÌJ³ŸJ4FGL J1912.2-3636?àƒƒæ‡'À3­Hˆ/À9û‰ø;æ`À;n'å".(@t9)ÂF6@§%?Tª?Ð^?ÜV?ϑ+6¯Æ@ëÅÃď@þü—À¦y?îÚ)'z¿ÕLÉè=ì¿éô§<‹Â¿éœhKBôq¿ëò`°
¿ÑŒ'Á)iUNASNone?çN±ŠBÏî?ÀZSÁ©=(?»ŠÈ ë|?µ¯E‰î›†?ÄÿՆéʏ?¹îiXëõ?é!Ñó×5d?Å3k{.'æ?ºƒ³,ò!¶?ÀãÎV±?¼m½4T3)?µn­WaŒH?ÝY"Â&¢ä?±	¾*Ây?¹†
žº?›ÚÏÿAŸ?ÜDè–U.›?¯º†–å¶-?Ԕ<š±.c?§Ðúˆ€?¿¶ª0?¦"•Œ¨-?`2"Î?°.Z xn–4FGL J1912.2+3621?Ö%Ç|xBÿ@'¬ì O*àÀ;˜Ø?ǖ,À<Ôe›eK´@(p¬@» ÒÞ_?Ü!3 ¾¼i?îbÑ¡GãÄ@
qU'Ù‹ø?þ:ñbÙ>?îAŸÝ€y¿ÓáP|ð§¿ÌËD˜¿ì·c^t)ž¿ïÿÞý¦ßR¿ï÷@s–VUNASNone?ãÂ;nG®?Æ;¶ßãÐ_?Âœ¢2?ºtã>¶?Îã¤Ü?ýOE×m?ÕûV¡p?Ò(
Š)7?ÙñŸT9?Ó+ø=' ê?Ñý

VÛ?È^,è€sz?ㄫËzd?¯I‹Ug°¬?ÈT†>œœ?§âIfÉéÓ?ÉäüKÃyÓ?¤¹ˆ7ª?Â]¨æå?¨•Œ÷ò«?äÍÀt ®N?¿*\Œ&^?Êk鄗2ã?¹â)e›—4FGL J1912.5+1320¿ïì²%+³?÷*ՖŸêÀ90‹µ«HÀ:ºðY|s@Ý$zØç@
¸·a+?ÇÅÿ©?ÔæÈ •¡½@àÆÜÈÃS?ýݹ\~0?é"Ë ¥<¿âõ:ªù›¿ç)ë‹Ô´ù¿ê^æ?d™Þ¿ïø~eET¿ïзþ^•7UNASNone?À^
5âÆÍ?´Ô
òK	I?¶•®˜¾?²ÐWI(?é%åÑ{5?¿2É¥R«?²@…C@Ý?¶ÄHN›?ÁTÙ)ý ˆ?À?ä\¶?ébÅäØ/Â?ۍ£…Fè?ì®xq±+?¢J³fV?Ä×Zԋ?¢ìÝR"ó?æ‹b^'?©Ú㻒‹
?'áI£?‹?zÛ!6qþ?Ì#,í™?¥ßpŠ³ãH?ê…õªÈB?§ —ï%¯74FGL J1912.7+4610¿Éë1¶JC4@/rÿÑÜ×À:Ï7Žâ†rÀ<¤¦Æ¨Æ]@W˜·Š @¬À½ÊÑ?Ŭï¢9Ñ2?×
;|Øæ@®0‡‡H^@0X,¼Ìz¿ÑŒž
²?ïcìÊì"¿á­˜‰Ï!;¿à—Lg"t¿ë!á1ßÈ¿ïÿý¡UûŠUNASNone3FGL J1912.7+4610?Ჟ(?Ä°|µÙ?ÙîӁº>?ĖµÁžP?³ÿÖò?®fâÉãM?æŽk•=Ñ?Äӗó?ÂþFD¶Ñ?À'+®üï?ÂÈ5dÄ*?¶gG1ì"?Ý»ìA'Þo?µ³uË`?×J›üzâ?¶.þdãžè?ÅòM\?¤&;0lÚ?æ1[©RŸX?ªœb"	xË?ÉO´IÛêœ?¨3Þ~Ih?»Õº!³0?—­iÐs[¶4FGL J1912.7+0957?ï1Ð]ô¿Â¡«`ìSüÀ8™‰!|QŠÀ9ÿ¦sœ¯Ï@>Ž2Þ#·@æÕw–?É;΢ºÕ~?×B-'ð
@~Ò`Š"S@Œ1>fm¿îô‡%ùŽÍ?ïÐý¤-¿åȪ(]\¿çò—a°õ¿ïrÂ)ۛ?±	5ô–UNASNone?ž%ýv?¡ßÂãɈ?Àɟ:ݲ?¾Š7ºè| ?êÜhRõPx?À½Gš–FR?"X咋
?¤ŠÌ
OÝ?Õ>ɂe¢¨?É´ÉÒÒÓÂ?ätw šT?ÉSð«,/`?²Œ1¥B?–_ú Fˆô?ËS‡¯w?¬ÓRCCÞ?æçäûñ
ú?®Ð©26?~€€þöŠ‰?k6zb?ÆU²| ¾×?°V¹äy?ê-'^Ùã5?°7
ï£û4FGL J1913.4-1526¿ëL"åB‡À'}ÚH¶R7À:¤$'–GÖÀ<ƒ¶85Ñs@¤¬é¶¹?ý+oðS?Ïd'œÒK?æðbžZÉz@‹&|k‹i@)WÅ8Ù»?ïéϘY(?ÒÝ¢] w¿»4J	Žt"¿àçÏAǺ¿ïùŒž^z_¿îTœÚ–¹ëUNASNone?ÑKŠÒ2f
?ÁݶUâ§?âÑ œ¿©o?Ŷ»r«ê?Â$g蜎'?¼mZËmr·?Â1%¢jã?ÁK}ufP?äç÷?Êó lôF¾?Íj•îTYE?Æýš*­g?Ä>;`e²?§Ÿ$…¼gÏ?娲4|cq?±1éÞA»?ÅYøò®Œ?¥8Ȭm£7?Ç0p¡h¤?§x"_v?á܂ª×1?¸ÉÒ¶µ—å?ЮÃqöQK?±úÅ.Ý4FGL J1913.4-2652¿Ô7½lóÛÀ0c÷œ"/¥À:ºØ´5&À<cAfҜð@ž«¼±Ì–@œ':×lc?ÖiÀãàd¯?ïГ*êU@؍]b²?öô¾
'*:?ïîj}L¿Ö´¯àÄ¿ê†Jg,_¿ïõþ~pH¿èup¾®ý¿ï‰:;e0ÜUNASNone?êÔôä¶?ÁÑFU?¥.uOÚ$X?¨o'ÔȪ?ÀµH5ä?½s÷FÔ?ÕõÐêÎÙ?Ò/ÐzA?à…GçB›?ÔcÃĚU?ÁÿÄÁöH?½ò1n¿€Ð?ßÁ`^Ðêð?²‡kÆi?Ð)ä…<Ë?°ÀåøÖ?лòIû?¬©g§*"/?¨ì,*Fú?šo÷©TR.?è³þz ?º"EYÉæ?Æôûu=Ï?µù'±G4FGL J1913.5-0923¿Ò÷tøò¼îÀ"FQ	¿À:?þ@_ŠÀ;œò™åï´@OcJµ†@fnŽ›9?Æù¬¿;>Å?¡ç®ƒMî?Û⍩K@ϒ¾^¿Ð¸W_bf'¿æ ñ—‡q¿ìðŽ]{[@¿ÛÓ&Á½¥¿ë[Ë}lg\¿£f_Î@UNASNone?ÇD±ÍªeÑ?¿˜˜—ü
?…÷&@NßÔ?µ´ãLKã?éÖöó"+?¿Ô}™ÁÎ?ãÒÖi ½'?É>WÜ®JÈ?h'pfüBç?x¬¹áOV?Ø).KðŒU?É#°Gyd?Ỿ~™šh?±éVFñã?§H\¦Îª?Ž/sùäç?ٟ×7ñZ?°¤^Ã*¨Í?ê²;ÜBo`?¦Tê4eTé?xŒáÑ­é?d>Dr˜8?Ävì'çµ?¦9©3öG4FGL J1914.6-1157?î.ÀK£Ü,À%È%žÀ:Ë©·À;'gÞ5ªÝ@¼3ù¬©Â@ðRãÒ¢Ð?Ì)³ʅu?Öﺢþ)@Oá|‡:?ÿՐx2Áž?ï±åàïïg¿æYôhI¿â­[þX‹¿ëA«"ªO¿ð?ïû÷"IôUNASNone?ØJÊYµi©?É!¸z¹3É?™ÛHí4q?–$Õ¿m?ãÀ‹»ªX?Èëe܊x?Ø×׿+ϟ?ÎÇò}Fò?ÀÔáÜy?ÃøkñËӅ?Þ½·¿ÑÂ%?Î;E¿ì=?Ò#exTºR?¬¥­åŒ¡Ÿ?Áà€ÕX˜/? ;Ø«8¾?âv-|Ë?­k"}?Ð4àݖÏ?°Ð~ðÄM?»ÿ¸AÐC?£¸-¨'kj?äe˜ŽŒÃ?²È€nÚB4FGL J1914.7+1012c?èÕ×z¥¸Œ¿Ý3qÜç!7À8ÎFèòAÀ:6Ô­kÞu@OîýNIå@•ÁF†Í?ˬâa3¡˜?Ð+ØËސD@	]5<ø®Ó?â8èDU"$¿æ»/€÷e?ïõ8áÈÝT¿èÛª¶!¿æš¶š[`y¿æÄI,«¿ï—ªÝŽ¼UNASNone8?¶µ.õí"?¿$¾Qü¬7?²EƸ U.?´9ÿÓ:­¶?êà¡J>B×?ÂЛŽÂ´w?›%H"4þ,?¤Ìaæ'Ak?ÏêKa¶?ÇêS¼àxq?ç,Bãzjj?ÇTOµ•°?¶"[ÓÁ?•hs¤…8?Äqwméw?¦þ‰µæ[Ð?è#mÒ9*?© >ë*p
?t½û"b|¬?bÉù§Æ*?ÉÒ'ðEß?²uM?‹R??éb$;)?²"JÍJ¥O4FGL J1916.8-3025?ÔÝaÆ&À2k‡	VÁÀ9ÀUWJi±À<2š†ÿ@ך¤["{?ü¡m¾I|K?¼((¾DÁ?Ñ|vžÏ@pÛjË?ùt(ì]`ٿ䇱°¿ã­¥àNß·¿Êf€Ä`˜¿Ü;Bö…¿êþþ"ZGõ¿æã"GþqUNASNone3FGL J1917.1-3024?ё­ek]Ê?¿èûدÀ?áå‡ð?Ä×Kã?ÅH…3
ª?¶\¥QAf?×Mi"à‹?ɏð	5±?Þ×Üuã'Ú?Ì<÷óüñƒ?Ä1¬A/95?¹ýè{9´?џØÒK3?³e~Õ?á'Í#œ?µ#Kñ(ÿ?Èg²5[.?¥i4˜8u‡?ÖÅScº;?«erÀ§Z²?È®BhC¶?¬µhûêf?Üã‹h#éÙ?²£—%"H4FGL J1917.6+2609¿ëBÎeܱ@BèbTˆîÀ:\p\‰mÒÀ;ű܆~4@šš"P1F@§Jº8u'?ÅmbÁ_?œš±,ç?ÊL齞\?ñ'ç[ne¹?ïþ.H‰Ý¿æ»áWžL‡¿ëÄþÍ%¿èÄ$½Nªˆ¿ÒZaueݪ¿Û3Üȃ<UNASNone?ۗâ†÷ È?Ée‹Áte×?‡¨‹'#®ƒ?®°Æßúè?áÕlŽ?àâ?ɇr|Vo?×Ȑ¿zJZ?Æ}ö†{×?›‡½Ž\9<?¦ïXbk¡a?ã?y³Ïù	?Å߀[²¿¯?⺙œƒHà?°«€WDo?¦Aèq
gB?pk…6$æ?׏¸×ÁV?¯¼>ËÙù·?âbi86N?µuSOfm;?—©9wUì·?‹xêKeið?ÙÀi–4š?µ…O•Ãœ‹4FGL J1917.6-3204?îY}ÔZúfÀ3*0"ÝzšÀ:CbzH›zÀ<*.y@-·qEèm@v"aKts?ÈS7_'·¨?о‰]aZ
@X/ž‹q?ý²-V?ï¹#!ÃM¿å]ñLÞÕä¿Þæg}'§ã¿çh¼LLí¿ê–`ÿõE¿ïÿ™s,ÛUNASNone?éÍù»plh?¸v"ˆÿк? ÉW¤ºò?›>"I¯Æ?ĕÃ)ߤ?¶zàAÈÌ?ëZ§~¡î?¶'!:üà+?§©q·Ä™Ï?©àFê'?¹V/B!?°KArFA'?æw‰vÏ??¯ð&ó@û?¸U!÷à+}?Ÿ"i¢;¢î?É÷Jþ4­B?§è†Zþh?ä¨ZžA°?¥º€#È¡˜?¸îov@ˆr?šdNú–µ+?Ðs¯3Zƒ?£'‹£Q=4FGL J1918.6-7813c¿ÛÆ7ÈÕWœÀ;æ·ª%ÙÀ:yl2š‡À<$aX"@ѧ*{ԍ@±ƒÞFqÔ?Ó@¼Þ˜&R?׈^2æ1?ûßFfìž#@Œ G2Ä?ï¾
'*:¿ÓíIå&_æ¿é´â_ܪ¿îú´|lb?з,<f¿ï¥c¯˜	UNASNone3FGL J1925.8-7826$?ìn6 Eì—?·ÑµÑ>o?Ãð&Þ-?»ÇÂg$?¸•Ðü뿄?µâ¤2v¨?풕O~¢‡?µ·e'T}ú?…áUqÁ?šzÃA`±ÿ?°¯*Õ瓠?²<Í	?ç)xw5ÍÞ?©Æ<Oé£c?µ%&àÊü?›ºö!n?Èً¸c?£à2MLA?í/>_"2?¢ÔÚ`öõ´?g¯
¶5¸Á?g@g¿
Þ?µÈ"–,Â?¢"b'^®4FGL J1919.4+1313¿çd¡w´l"¿µàK¯«ÕÀ8YÂÅ+À9úád3†?@ïf£M!œ@w$ÄÛfÄ?Èڌ(õe?ÞUœŸ]}ß@žK¢•Áž?ÿQünûá7?ïï>ÜÇ?® ÃDõ1¿è'âôV¿íœáL¶'ø¿ïÿ¥!b%d?ïøDRëUNASNone?³1Š;''Á?¿ym[NTó?'+¼Áo"ù?™F f
)ù?íp҄>à?ÀfäÖU>?«$H
3
?°»ûš%Ò?ʚäëùú´?Ŏ§"2=?ç§DYn#?ÆHf]jKú?£R°?$ÿ?¦Š/A3²H?ÅT=fðQd?¦Üеyž'?æú4"f?° 6±	Ë?rÂªzf1?c*ÏИÏ?ÊðO"ÑÊÑ?µå~ڏ¼?éʙv˜?¶"ƲüÚ4FGL J1920.0-2622?åç}€ðf–À1"ÙºÀ:MV¿)vÀ<V'Tà@.ô®¾@I}<kÁ?Ç׫£Ì?Ò¡ä@Ü¿@
ª"Àā@4æv"1?ð?Ð'UØy©¿ãŽO¹{·¿åÀÌäIÁ¿ìˆ[NoÑ¿Ñ&w ÈÍUNASNone?ßñ1™sûú?Åÿá…r ø?Ñ ¼m,¨d?ÃGÝ*[f?ÌÜ#ò¾·D?À**֜RR?è¶Ôæ¼q?ÂÜ3ۂ#ª?ÀépFš?¼ÎÌ҅æå?½ä<éH?³ÌWÏ0N—?á=þÿ¤ç?±xnñ??ǝ#DàP?¨Ïs²?ѵr)Ž#?©©³»šH?á¢ÿ?ÌÅÕ?¦Ø$Þh~?ÉóðA‰]è?§ƒ"Æ«¯E?π¿CŠÅ?¦€ãj^"4FGL J1920.7+1334¿×qAJ;ý ¿È‰S¦EN"À9Êc&3À;vރ®uÊ@/ Ô ~%@Á›@bƟ?×ÓDç:·?ï•ÆÁ#@9Ë@D†r'&?ì®rn²e¿îZièÑæ?ÀË(²Ñ¤¿ê€ïHø—V¿ï÷Ú,0às¿ïÿüÉï£UNASNone?µM>}ö±?²‡‰«$B»?º
ë€Ë3?¶\ÕÔ×5?êúÌÐ'Ä?¿±ÙÍʱZ?¡`'€Ã'T?¦š¬}.Y?Äz'z¢Œ?ÅÀ0˜Éé?éËXéK$Õ?Ōþ®?Äy©óUo?£^|Cî•&?Ȟã}¾«ß?¥¦Mz†¬z?ä¹Ü£ºù%?«æŠOS'­?•¿UTd:1?"4kÔÿè?à…3ĖÁ?ÂöºUœ«?ݙ¤Ÿ0ŽÝ?ÁÅ@ ½Hò4FGL J1922.4+1453c?ê¹æó…Z?­ºãôº/À8ɼHKÀ:%ç}R@ó¨9Dš9@©K£l3?ÐTa¡Z®!?ÚAœ¬s'@‰¤Òh@
‰ºr¿íxÚÂXՄ¿™¼S`'Õ;¿çJè3FS¿êÙ๨¿îª,ŽÔD¿ðUNASNone8?Ñ]À/6"¢?×/©X^ÿë?¢1âŠLï?­HÏ-‹"Z?æ/üÊ<à?Ömðªwê?¡§?†]ݾ?¤I¤ªB?Á®I@ud?¾>{34¡
?ê  uJË?¿ˆßt-ѱ?²ˆ|=ö?'~J¶ý?Å7úŒò<…?¥&áH?è`ñÕ#N?§·ò2³?€Ü؍š€?nŸ'g_?´ëã@˜Þ? LX¹m{°?í5Æ"ã? ßôø`Z4FGL J1922.5-5233?é"'.ÃÀ9͋¤
âÀ:w¢'^<À<tñ´âg@ ÖQ…Ú@M œÃ?Ç6E¡ÊÀƒ?Ñ2%acr@@™'6@3{ùö{?îú÷íâÇ
¿Ê$ï"¸Ó¿áæüŽ[wö¿éC>n$Ì¿ét(%¸÷-¿ïý–-ÔN¡UNASNone?ì€Ì)ÒW?°p%24ƒ?ŒEeÞqÉ(?ˆê7
"¶?¸pòZã4!?®ý²ÌU?îB´œÙ'?£pŠVB?|%aa/™B?†Lµµhu?¨Pês¿? îÚB?ëuæIWù=?¤'æ}Š›é?¤ëý½‡XZ?'hhÍ¥'?¹ÚÎÖ|‰ê?ž'YY"?í\Â[rBÍ?­µµÔ?—Ô9(˜ ²?€&ÝØ}ÐÒ?®I½´ÂÕ?Š¨EÞÞ]4FGL J1922.7+1428c?ãYx[O¿ÊGBIP«êÀ89Ý3L]§À9†2Áô+¶@¥¿Ü#å@U>Lò?Ê&n©«àn?ÙÂÓº&×Û@ý8bGõ?ûvýz#Ý?ëˏJ‹>¿æ2Ï˄Î0¿â•ýÍö˜x¿éjª}ík©¿ïÿRáNd?ïÆ+B£éUNASNone4?—³5ãw‡?´Ha]B.?'c‰S£?¤wc­eUŽ?î¯M€GýO?·	URÝr?£QR"n³¢?ªëyš'^?À'}÷W²?¿ß<(Ø?êªKYò~Ù?ÀšC»³ï$?±Çc1N?˜®ô‰o?Ê@€28f?­§N¢0ù@?çNGE€O?°Ûö¹‡õ5?PåƐýÜu?G]l‡/B?®ºd˜éð´?Ÿè0èx°?îæÓ(â? Yª)òÒ4FGL J1924.3+1601c?éºÐÞªDã?ÉÎ81ʨÀ9uk¼ç|À:UùÖñý@ºE?Ð$›@8圧k?Ñ*YÛ=¨Ø?È.1× ì@IÄo0:?úٔ¾¾l7¿ÒñõNÌ?ï½Ë½ƒ-ǿ燊£\'¿é´ãÅ˜¿ãg†àzª¿ðUNASNone8?Âa0·¤ü¤?¸ •n¤j?°¥"퉁?°öh`ÕV?éSTt§?À-'­xª?œ˜§]Í? ¤|ç˜BÅ?ºZ}5þî?¼ù$lƊ?ëߌ«"3?½·Ô÷ß'?Á$	™Þ¤?¢ÁgωY?À¥Ò¬¨?¤¦·P•3Ï?獉4î^U?ªª»"*B¡?—»ÞØgßÈ?€Géڕ)?²ÊøMü¢¶?¢GP[[¶?ìèÁÿ},«?¢¬ø_tt4FGL J1924.3+1628?àIP!f¾6?Úb<5:tÀ:k÷ÉЙ
À;'§WÈ=ò@#¾%7Çíj?ö·zU0³ý?Ñ£_ Ïmç?Æõa€ùd°?ì5J¿ì¿†?øߣ¡…KY?æt$'/¾¿ìW<'<ZÏ¿ßhŠãžJƒ¿âkÂ[YÂê¿Ù驼ÒXÓ?ȳùAI÷UNASNone?°÷
ÒÑ?°#½¦ŽŒz?_–†—H?[gÚS‡†?íёØÚ?°G'wê<´?­¨A|Ôê?¶—Fi2* ?"…^ésJ?˜<M2]
?íÓh°Bf"?·wh‰t÷'?×ÃÞôsr(?±"fPIÒ0?¥_wm'?‰¿L™è™?âÍ¿ŸÎÐ?±
;v=€
?±í·-*!d? ·åœ¯£¥?68|b¹?aâØJ!.?íƒÜª;Ã?¢\¨+b©£4FGL J1924.8-1035¿Ûÿ#ârÀ(V>ò"{À9۰݂ývÀ;éü7ôc@™ÊM²o@Мe%õ?¯fõØ^Ñ?Þ{üOÇ>@>+ —ºœ@áù&Çêæ?ïé‹$£M¿ÓgÃþÇñœ¿Ý@`") ¿ß
)N­âý¿î'x_7H¿ïþ!†ù"UNASNone3FGL J1924.8-1034?"H±…œÈÅ?•‰T*H–˜?î'ö")|±?§Z½‹RøÎ?›X}õ3¡#?|ʱÄ?²+lÍXÐ?²=*XÆ?鑒ޝ_Ì?ÁÁÓYÿen?À£þÞrg?½$=F+*A?¬ÙByšòƒ?—.:Ä÷<?é
 ?©Û;º;lo?ÂUQpÄá?¤º¯5ºÇ?©ûЖè‰ç?Šë«1/?áS79\ã¼?²aÏÉÔ'?Úzi'L?±dÆå4´4FGL J1925.3+1522c?&Z¿Ô"j…¯×ÊÀ8ۚ<VÈdÀ:@æp–@òµxrW‹@´ØŸhæs?Èñ7¥³®C?Ösâû¸G°@‹7T*?ÿ'Ú7Äg?ԊÿbvAÑ¿æË ýP£¿å·cyL8¿èàyAàJ-¿ð?ðUNASNone8?ËGü'èÅò?τ¾R'B?­–•Ç?°h>xj?ç]Çsue'?π©i®ÿ?²–ý´<2ú?µ"Bú'W?¹ªˆwÌ?¸XÿÙ@@?ꉊøi–È?¾9+•ˆl?¿2þd>â?£ÐÓã¾D?ɪ瓲
?®ny÷?å¯ù˜Ë¡?±-&Þ4ý÷?ˆù|ê6É?zñ…5¬z?µS˜Rè3e?¢´…´†R?ìñ§‡P¸?£ÚŽÚ¯4FGL J1925.4+1616?áò¶'¼)?µä³HlUiÀ8+YhQ"2À:1°Ÿoœp@ @Ÿµ½f¨@ÈÌW\h?¶DË+­?¹=§UnòQ@Ž­…èÝ?ý´ý2p?®?ÅdÞ{öÆp?ïÊSá(¤d¿äV5@Ԇ€¿çÖÔÃ;S"¿å;$,/3¿à+Žž¾Ç{UNASNone?¡éù—°6?•#Š+N?Áë"<÷Õ$?Âæ×Ìrç¦?êm8Ñ(´?Þ4ð?"Ky¿OR?•€l3ÿ‡?ÇÞÀ"°?Īzïh@?ég­Fƒ?Äp]"Ç?²gÔ=ýÚÐ?"CjÄÒÞÔ?½ìTÃþ±?¨9 ݍ{.?éõzßÀn…?ªM³>G&-?›ˆ÷©Ù?Mì¤?Áæ­ô?¨üjæ?ê­ ³¤ý4?¨	à¾~²¢4FGL J1926.4+1602?ä;ENÏØ¿Ïþ^Õ£`À8)çZÍÀ:*{¥t@^ŽÄÔ[@úv¾£>^?Âiž1Žm?Æ¥˜*ƒ·/@
‹}ý[àÑ?üÙ,|4ÙÑ?ïhD¢qYŠ¿áhÈv%÷¿åeŸ—	œ¿æñÑiÀ¿èEþFÂ\1¿àúsÅÊzUNASNone1FGL J1926.1+1601c?–˜®	þî?€·:ÿ?»Á÷rLs?¹óüˆ™Ç8?ëÒû¡n9?»Ê³Ä^?	0åú	ò?›P\VŽ5ª?²'*•	Å?­ãÒÞÑ}?ìő&.÷?°NÅ!:w°?³NW߆Qm?•ÏϙУ?½‰acÒÂí?£ÏVÕfI?éåהÝu?§S6š>ä=?'øŒÕsÿt?m9Á–Ø\Ü?´Á÷ú°Ô?—E‰óÖB?íÞÍfùç?—å "D…Ÿ4FGL J1927.4+0253¿×'¶ú†!À·tî¿eÜÀ:nš»É.À;îjCk@5w>Cˆ@GEÙþäw?Ñk€'Í?å{h÷:^¡@tu½ò>v@~?NI¿Ù|½ÀÀO¿Ö†/¤³S)¿â2•"´¿ë u¡æv¿ïÿ{Ûèt?ïú!Dô&UNASNone?ÃTÌ(%ܜ?µpUœ0ã;?Á?¨Ð€óà?º'§9z­Ë?æÚâÁÖKá?Á4´rrƒì?Ô.ì~Y)?ɝ aû?²ÄA8ú¤Ž?¶´ë><‹q?ã/b¡~Ù?Ê `‰×?Ø_"b\a=?²a(1"
³?Ðý±Ë¿Š?±o\†éE?Ö£+Ñä¼?­ìû¼£Ãö?ÞþÄ_ô\s?µ#[
Å?·°|ì2¼? ´%BöõÇ?Ûš–Ý?µ(s_7Ž=4FGL J1929.0+1729¿è«=Ž‰xÿ¶Ÿ_´ÆqÀ8<ó˜:õÀ::&¨á5:@Tó®N@ ,Æ1¨?ººdë<#?ÕPâC5à@ôH!ˆ@+sxó†Ë?ï'ÞŸ]'ù¿Ö«³¢"NÚ¿ä¶b'$-¿è†"Ú8+¿îDl@šúÿïÎ$ É8ÄUNASNone?"µ–U|'#?€R(èÈË?ä€ÝÌÏÁ?Çö
.¹×?ÖX™%º{ì?ÆãñX‹o?Š/Öå?1?'=Š3Ù-?×ç¼'T­Ì?ÈñW»EW?ã•ù,ú?ÈöÀlu?¨m6©fŠü?—8Þ3?ã$
û+?¸Æ°õ+1?Öĵ8L?¶«×€Ì?hä±|wò?UVÀs?ÓZ
ë'.?¯Ìz.Óô?æ:GŽ6ò?¯¶;Êë	4FGL J1931.0+1754c¿ïàõèò>ĿӆoE],VÀ92ð¤BjÀ:‡4éد@ê''¸@_Ëâ˜@(öÎþÖ4?ÒÎBXõ»@
…凮¶@öˆþð?ïë@öjU?âA¦=—¿çuݜþ¨è¿çdœ,ý¿êϯj¼6}¿ïý "DsUNASNone8?×
ó›åÃÁ?Æ8Bá)Ç?Ú2ØxÆÿ?ÌÙÑ,ÃX?̈́gÖ¦y^?ŅÁKŒª?´íã2ƒ"?ÀE—*"ƒ?ÀcIo€½à?ÆWµ>e˜?éIq=Ï^'?É<s%Ê ?ÂË`Ŕ1É? ½…m~?Éߤ°½Ü?«!—dBa'?äÕ>¢k|‡?­ÀØ£'÷?˖Ḧ́®Ä?˄:_@Â.?œ¶ÐtX®'?¶xum¸?è4·HüÚ?Ìë¥÷}ã4FGL J1931.1+1656¿ã1 °}ûr¿éew•ÜvÀ8k§AøÈÔÀ:£ùnì@é'"§ŸÂ@蓂(cÌ?¸3žèãÙ¯?Øf¨@%‰ý@7Ý÷vÅ?ùõzÞm‰?ïÕM9Æö¿ÝËØü0Á¿ã£˜ ö/G¿é ÝDU¿ío³íöz¿ïàåõ"UNASNone3FGL J1931.1+1659?‹ø:¼?€7S³Š‰?è¬B	Ys?Ÿï–è½?ÌR˜>àÄR?Á¹m".ö?…?nbë?Žtׯp?âQw eMi?ʗ3_Z,?Ú³#ÂMÓ?ÊWw¯zB?—ÿ	àºJ?…0¶ïŒ¥P?釜wXûÎ?¯bWÍP…?Æá­Ÿù?¬Â	ê#?VÌ2NÊ~?Aì,OImv?Þ·þÑ
q?²là§xîw?à˜À±` ?²nîx_ó4FGL J1933.4-2711?ì€å¿Ñ«sÀ4§ã\[J©À:]«p_À<€»|Bq@k"§ïó˜@)ô?Ø]$?ÈÍfOÀ1´?ͪxúgº¤@à±5—''?øÓÁñQ'm?ïøU¦P¿äó~¢r[<¿ê_ý@²ø¿á'–
qH¿ïûÚ×Q‹
¿ï`낚y"UNASNone?íÇ÷y5L¡?ªÑzf¨?•
tCÀò¬?™9õ°>½ï?¨ûNJ'¢?£a¡Xs%?é$2¤¡ö?Á¬µ½ué?¸-*…Ýþ?»Á	 _?¾BQ@UT?³"TM b9?éåáØÒm=?§ãÞRו?«æÏÿþJ?—¸ºMè?ÁnĜ¶¸†?¡bò8T½x?â«ÑÍ(w¼?«‰°Çµg?ÈwV4êF?ª)cöP1q?ÍNAu)6Ë?¦1E,¢¼l4FGL J1934.2-1446?ä(_»ã«À0!BoçÀ:ײãâ"À<]՞,¦@KßS75@ôK+w}?ա‰?ïúºEዡ@©¿f²¼€?òJ̌¶b?ïûÂ^ôÆ¿âI†[Ï¿âp&¾°ªW¿ïþª_ºz»?ïÁ5Ø)!¿ÛèFۆ£ôUNASNone?íήò©o?µQè±ÿ?–´ú?§LÂÚŠ?¨}s¢?¯&O|6¸¶?æ'bûN)?Ð;,Q^Aâ?Åjé:h?ËÎÚõB…l?ÀPY*´_F?¿¡è°"µ?åW'­);)?¯gÏTR?Á2x¿êÖ¸?¤Ã®€úDÛ?Éo|‹p<¥?¦âwjì>?áù¤†Vÿ?ÇfCAÎ?ź«ÍÎ?Çéöå?Ñ/nÐqƜ?Â@]à%á44FGL J1934.2+1036¿ïŸÔì½Àdf±æÀ9ê¡/"À;q¨žð@u+'SO@êÓ²š?Î8×!qÍ?̪'».å?ûìÓi©@Ú!« §¿ç¼uÁù	A¿âŠI{õ¿ç«Úy]¹ï¿ç!¯}0­G¿ï÷ä]b0Í?ï(ڟsMUUNASNone?ßcñE'c÷?Ä3gáŠ:?P–(ø?‡=âÌ^Ú`?ߚ±‡?Ä1L7Öµ?ÙÐo/"ªO?Ë#ä­PîÍ?ˆÃXhϖN?—( $gÞà?â´»'l€?Êê%ŠUÏ?ÚÒrôà>?°/¤DKúï?µÒnœ+O8?•‹iå«a?߸ñdó?®íÒ§®‹?âûug²È?¸ÏHcóT?'S¾4&Äw?~§õnOh9?ØóÙN .)?¸¤——h€4FGL J1935.0-0553?ØOn&oÀ(¾Ÿà·öÀ:(òvªHÀ;­Ëwb7-@^R 3Q;@Ç>
&Ê?ÌVïûÐñJ?ÉÀœþ('?û)¢á@ø@ÊQŠŒ5ƒ¿åu¿äF¼¿á"՝U漿êú©]\¿âSÓ¡Ó#ÿ¿ïÿÿ" 5•?ïâÞA>c¾UNASNone?î¨wÖû—?Ÿ¯ÇI?ƒ"'4Ú?')™™bp? ¯øÑܐ?›C3xÆ?î	ûÑÿÊH?°µºÙÞن?x™ÆYŒD?ºŸOó?«nlø`?®Ïu_u?ç՜!>öè?®ås"]¡g?¨XàÞW¼?'çwÇ*ò‹?ʓWCnCð?ªö6ڕU?êýN—4‡V?¨Å‡=&'?ˆ@Zíe3›?vÝҀÿ,?†¿ôWm?§Þ[­N4FGL J1936.6+1921?ÎôÔÞi,i¿è°IáÀ9"+zMÞÀ:µ®Ò­@Ù£‰²pÖ@€"Þ?ÉSàQäÏ"?Ì%=§*{Õ@àÌ¡-â'@Òÿ–ÎŽ?ٜ߯}‡?ïùRژg¿çÝgNòr¿æj}2…
¿ïþ;·f3?ï±<î×íUNASNone?͕.²'?º?†³g¸?ÎĨŽÙå.?ĉi¤"Úð?àéqÕ}Ú?ÇNÛœ±?º8&Ÿ!ÿ=?·é¬Ú¿ç?¾7ÄnêÄ?¼9z~·¼?èò«Mâ¿?ÂM2ª#%?ÃlHP$¦?¢Ë¢"³K?ÃðÐIÕ&?§Wëäf?æ(Ǜ¦A?­U—Œ:tï?¹ZhÅj+? 8äÇ
°?Æb]ÖÕõ?°?ŒÇ"¹Å?ç<9[q=?²Hº‰Û¬4FGL J1937.1-0444¿é5K±Ÿ†À(¥îÇÉXÀ:§
ûÅ<À;בÕùµ@ŽÊɽMÔ@Ñò¦{)l?ʞ#×u;?x	‰k¤ï?´!ˆ¬6@5™ ûb·?ïO5'‰ ¿ì¿ôÕ÷¿âѱkë¿âLERðgÝ¿ß=W´¿ï÷ˆ—é–1UNASNone?í£O•DM?¬µñÑÛó<?tzßÈÐ'?q°yª@Hv?±¥;§á
a?«Î4<ú-È?ë.ø?ìèX?ÂâòXAr–?q©ÜZô¯·?'ÿìÒ¸y?¶Ðt¹?£»Í´?è'/âÝL?¬Ps]r5Ó?˜ˆEaº #?ƒ^
ó<—?ÉÄ"=6Î?ª©6\	l€?åt^OZòC?«˜xúîàu?zçßéO˜?jxlч%Å?Ô«£á¥ª=?«j1»êmp4FGL J1939.7-1242¿³ä77ÿ¿¡À0`À½ÊÑJÀ:OL{ٕ2À;äñ"«=@ã7sá%@÷>^‡?Ï"/)ä*?ԏ=?{•ø@VÿëJ?òoðJÖ=?ïá·uL³7¿ã¬u:'Ä¿éb†ÝÕ2Í¿åãÈý4s¥¿ïÿÕ} i¿ïä×»=XPUNASNone?íPž‰ ã?±ÝQïäG?›ð¦¥¤¬?¦vòº?¬ýÊěí`?©{Æ"'õ?å®æÄ]<ß?ËÿýàÃv?Æ_šŠšw?ƚG'££?ÂåUTr
?½ç°›6§¨?äHæhÈf‡?°ŒB"t½?»¥£í^?Ÿ¡I¸?ЄëçÆ7œ?«Q	?Ò@!YV?¦tZ+-~?Ѓé
é)?¯ø.'{`?Ý;‰ñŽ?±7*ö¢ü4FGL J1940.2-2511¿à¸û-՝£À5[«!ZÀ:61•¤A"À</Æ|P³w@Œ8ê8C@ZمAóÀ?¿ŒãÓ¤'V?ЀhûÂÄ@·»Ã
@%£fÌè¦?ïщàiÝ¿»Ž>Wå«¿ãi–!!Ë¿æö.Åæ(¾¿æåP¡F6¿ïÿÿ" 5•UNASNone?èNº·IIW?¼ìøûrGÊ?¼iÂ×pÝz?±üü΃ç?À3·"kå?²hˆ'ÁR©?ê9Ø "ò?½¬Â[¬ó¯?²ýݕ©&?µ-`ÈÇø€?»3^q8¯N?±eT BÖ?çO»%•V÷?±‰ð‡®àÉ?¼\îøþáG?¥h{ãM?Ē›í+3?¥ðqÀtÃ?å_)ýW¬b?£Ç»:º•?½K	iÓæÍ?Ÿ¾ìc'Œc?ËÝÓU·[?Ÿ£}:\iÝ4FGL J1943.9+2841?͛B­	õ@!‹zՉÀ:—{!ŽÀ;ú¨(÷@UÕ¢ß="?ÿ'þtå…*?ÒM£!Ø?á÷Ix@æþ*¼l?û?P"]?è¤zÏ)¿éS-Ú-Þ`¿Âë·sŸ4
¿å0>·ç¿ïûêAQÙç¿Þ»k›¯svUNASNone	?ÑØOxMy!?ÀWj["?¼C+TÚb?´¤Þ;z&Ý?ã‹rÙ>b?ƒã¨M6?Ò*®ËÃ?ÍÒEJð?³S`@c	?¶J­"J?ä€<ë½?͌ȑê`?Þt>ñÑ]t?®éW[Ôn?ŵX©?¦Ë;óf?Ö±¹£¡?«‹¡*º[?Ñ]E]aý?ª"Ô(¨H?¼'És‹Á=?£ÐSû˜B#?ã¿$#ÖÙ?±îÎÓøw4FGL J1944.8+4301?Ã
Á†êâ¯@"ˆ^	}À:ߝcRµ¯À<®nƒkYë@š7›Í¦?ûewS´?вï«ôæ?ÝßÉÿ'ò¶@
°Ð?Hl?ð\^š/A¿î'@"ªt?ïý%Ÿ÷¬Ÿ¿Ð×L¶8Œ¿·ByLG+c¿ë4rÞn೿ïÿþ½à ¿UNASNone3FGL J1944.8+4300?æúìÕC?Âê#?»´¯¢-e%?´Är õm?Æ9ôÙÜíV?½ãp=Rû?Ê(%÷jÏ"?ȂÓ(Ièâ?Þ@ZbŠú?ÐÞCbÈ®?Ô«Ñ©è
v?˜'¥zù]?㊕UÍ	Å?°â=Ég?Æø†_ò?¬h'ŽJË\?ÊݘŒExý?§Û	H£Ž…?Ûz'2Iµ?´ÉŠ$aß?×b35FçÁ?ºàåSø?ÊGz'
?¬¢#3¯°|4FGL J1946.5-1527?îÕ}J1IÀ3ªCåÀ:­;qÆÀ<2©ˆúåå@+QœU@MdQ¹08?ÌZÂl½?ÖÂ{»[@û͆00I@$_6œIL?å*zAå}ž¿ØôKâ»'¿ÒЖ‰B¿ä¶ÌR֒¿íÈi[
lпïÚ/÷>_UNASNone?àµ
XVõÏ?Á¢}à/Ý?ÉîžD€$R?»íô?ўœ-9?¼5#"˜?êBŒ³Wã?¾8Ÿl{Œu?²1}póôœ?´¯^ÎÛ؛?»ºö‰LP?²u5§TÚ?â8táa?Û?³ÚM^#?Éޅcp¾?«ä'ˆðp?Í?§hÖ?©Z¤a‡Zu?᳀4㶷?©\¦†ÐÕ?¼¶…zɪ? )UÑÜåk?Õk^7†Lf?§Ç¿Õ¹ÿÚ4FGL J1947.0+0031¿á@–wj¡À(2¦Òg@À;KÍ]ìÀ<±
À¾¢@Ͷ˃¡‹?þˆKBôqW?ѧ+='¨?ãŽYM= @º2nU"@ìé‰ò?ïõ-¿‰?ïý¤ Y?Ùς‰²›É¿Û®âÛ¬ä¿ê¬í3t¡"¿ïý4©Tø€UNASNone?ç%Û!?Åòy1Û« ?̚v žw?ÄÔËU÷p?«DfoÕÐQ?¨Q $qÁÚ?ä§ÅÂdã?Ëå
¹¹ÃT?Æ]¶øcr?Ä7i`VIm?ÇA‹@ê	?ÃÌŸc?â9ncŽ–?·*
˜ÑRS?фÄÜx¨?´üä×6CÊ?Ä:èØ\?£é¬ˆòq?âryÓ±?ºU/gß!2?ЫúÂgž ?»P¸Vv;?ÆB@"ä¿û?¯ßcâì³4FGL J1947.1+1729¿Ã˜•£íxÀËEˆ MÀ:~]yWÚ²À;ïpx8 @YYJt@ˆÞ{Jùù?Ò¢É4<?à®
>¬ãù@&Á» ÒÞ@ªåq^?ëgÇÅ&^?ïÍýº¿Üê¥OÛ5¿ßŽØ'?Ù¿íÃÌ"'áÇ¿ïéý"ë´ïUNASNone?Ñc·KÔ¨9?¿ANøÈú€?¾Oٗ•QÏ?³ã+zŠC?ã")'#ª?Áӗªy?ÉÖ¸X–?¾³EüIÓ?§A6,ê«?­s¼w}?è>‰'¯v?À ¾†¼
B?à³ÄzX?±2¨j®)Á?Äú4úU^-?¤³ñ<–ë?Ô]Yà6;?«ÃÁ—!Çô?ۆ/ˆ
Tñ?°¹i'âkÙ?Çҧ̡?°&>è©?ؐ|îZ"?±?Óõ™…4FGL J1947.6-1121¿é­PÚ|Ò}À1'à°«À:&whiÏÀ;ñ"ï¾i]@LAô—2@÷T°[|þ?Àò1uÃÑ|?ËÚ\S=@áÝBeÖ@îa§ºÅ?îúA¯Í¸…¿äÅïbùÊ¿ä˜zJHùn¿ä¶"¡¸!¿í6A
çI¿ïÿï0l¯UNASNone3FGL J1947.4-1121?àá"}J?ÂÕÕ¿ähµ?ÑV:}~Å?Ácü¦ÈÇ?ÉÍ=ÕÜÔ|?¹(
7§ü2?臔¤eþ?Â,_E$œ?»%ú<pe?¹?Ñľ:?ÀXšqMgÖ?µà£±ðqç?äšu{€8?±0G÷ýY?ÁRÓÀÓá?¦óŽð"Eá?ÌCW
+=?§¿c¥çæ1?؀çöØCR?¥øäø%?Åí3'ë:?¤|þˆ?܈~ˆ^Ç?§gÐ"4FGL J1948.0-2845?ä¤Ñ{ª"À87÷ß (À:Âôí}F}À<'øxLAø@õÉ¬²@ÝӅM²:?Ҋä?Z2ü?ÆÍyÛc='?öéjâÌéR@vMP¦?ïó÷H¡Y¿èM!@—tÑ¿Þwgà¹é›¿åá*È*§¿ð¿ïýl§ÉEUNASNone?ïPÓ՛K?Ýìög'?s}t=-"o?v[zP|uP?'ˆvMþ?ŒÅƒÖ9%­?î¡ ¨ã}? 3¦c±?pR•^NåÏ?}#@Ü?£ä›I§ëy?06QÚF?ìE½7,@E?ŸÊ7Þ)Tr?°%èzt?‹Ø[-Éì?¶ª=#ß8?™"Ǡۅ"?ì7ïŽwñÒ?š¢Ö4ãÓ?ƒÚËýt\?rŠ)z·?»Å@2ÀÂç?™»¢ùÿ"$4FGL J1948.1+2511?ÕT÷Ëu.¿ÆÆ»üXÀ: !}(IËÀ;ÎôX,@ŸR–$ð@L¦¼—Ëc?Õ¶?!}ÿ	?ïý½À•[ò@Ö|^p@'ܾ²X¿îêÎà£Cg?ïƒP˜È¹¿ÂTR½'M¿îAŸÀäa¿åË@¥â}8¿ïþ½_ÇeÛUNASNone?ã3]Müq†?Éúý	Q'?»øU´@¸?¸þ _Áû?қ/÷ŒÅ?Ç]¸Ã,aN?¼¬í(:Ï0?À»>%¬"O?ΌÈ(Ñ1?Ê 愧Î?äÇ\hîqÏ?ÍÆr^'j?Þ͋àÛ5=?²<ËA"ú?Ä9"!'?¦˜v
›?תH?°ïmV¬ÈB?͗Ús5?²G«óéj™?Ýî:Ææè?½&}~ß.?ÓEüµ«ß}?·rÑô¿ 4FGL J1948.9+3414?í‡óç˜Õú@ùÉÕ¡‡¥À:Œ%ÿnÀ<d._ŽÛÐ@€Pþ .‰@'ƒ$ã?Ì)FNm÷?ã$"¯&ɘ@4·|Ùor@*¥"8äù¿ïþ1ɦ§Ÿ?ïÚÚ¬‰`f¿Ï®öxçù¿á©=¦~¯¿ïÿ›‹â ò?×Fë¡Ï4UNASNone?ÑË[Î7wH?ÁoL­e6à?áËÕØll÷?ÅS¢Ðrh?Å9ñß]–?¹'W‹‹Û?ÎtÜ7†?ʨçÓ´_?ØlC²¬½?Ð2¤9Xa?ؒ5åÈ?Ì|âL
€?ΘÖ1ëų?²)]ião?âÉag‡Õž?µíÊ6ëž?ÆA¤/ôã×?¤øsÃýJ/?ã—%²"Ê?±WRJµM?Ðgæ£=?°íKÍC?ÃÖ#œ^?£éÄéC4FGL J1949.2-1453?ë
Ôæ±À3c 1ί%À:9ìTRÀ< 5)­x@584¤ÍT@º®ƒ?Â-æ˜$ú`?Ïç™Â3k½@
®Æ±@£'ôf™½¿çXJCðñ¿Ö·_þs¿ã
çŸïõ¿ã9>Js¿ï¾'€p}Á¿ïûúëÄ	UNASNone3FGL J1949.5-1454?âøUÊ)?Äõ+¢
Œ?Ô®?'OT?Ä.é@Ì?µ†h´qf»?¯X³>£L?æ»ðnðz?Å­äa4 À?ĂûBËaé?dºÀ›'?ÀCrµš?´»©gªûÖ?â6>!oÔ7?³\?ÀÌª?ÈdI©pƒ?¬){!f4Œ?ξ[—>Ÿ?©5tZ·?ßc5Ÿ†?­4C½W?Ç4@Ċ}?¬vµi©š¸?Õ'Éþ4°?­u2Hnv¬4FGL J1951.0+2523?è:ÜÀ"a$¿ä¿Ž‹HÿÀ9á8ˆÝ‰³À;‰á<ÆYì@\fHß@´±'Äjþ?ЅÁ?ÐÐh?èlŠlÕì@ûà\÷R@½çMVŸõ?ïðäÚ	Ì2¿ßöP<Xv¿Ó&íàBËW¿ê»Á¬Þü¿î*GÒ&©¿ïü UŠ÷UNASNone	?¡]
¹B?–ÁaL½?Ôo̘ÈIœ?ƕ	›S«Ø?ä²HعÑ?Əw^L}j?¥­8EIö?£5=Ê¢M?ÆO›§ãÄ ?Âŧjl?éE"Rº7?Á½,¢hœ?»ÇÑþ ®{?šqØeDõß?Ԙ#w¹XÆ?³¶"'Ž??â:ôO=Î?³Vj¨ó¥P?¥2h¿?‡Ñם†Ï?áŸ)…ÃÆð?µGz@ἄ?Ú_äWÚB?´½3B%½4FGL J1951.3-8015c?í2ˆZÀ=;0aǛ5À:P,á	š³À;þí¢/jQ@p*^£N@(ô€oüè?Îå?	U>?ÉsN@Õ³%?ùи´çÓ¹@Ù1΄1þ¿è"Xº¬8Ù¿ÞNvZ¥=¿äÂAƒ-¿çÜzŸƒh€¿ïü»ýǖ'¿îì:ñm–UNASNone ?ìl³€
å?µS@²–U?‡|R2ã?‹Þ«DDïF?¸étug??´iâ"?î|ûp–?§jü_€Ñ?uÞ;"[?…*ƒøä?«"½½–?¤ÈÈs‹Ô	?é–w¹r²é?©c}†">?¨vhöÅ?'¦QY"¤?Ã¥C÷ƒ?¤™'¾€e?ëüéÌ}DÏ?uáßÇÞ?{1M¦Ý?{eÖ§ˆ]Ñ?¼iNÕì$ª?œMg%ŠæÊ4FGL J1951.6+2621?ï{Ã*?L¿ÑTËß<'À9=kŠ'•™À:ÉV¸syt@‹ž[JS‹@ÓQùÇכ?ÅÔ\c-L?ÑÀª?.>,@U-úNw@#^邏?ê_åBåWÞ?ï–Ï)ž_¿âcž\vù¿ëN
>¬ãù¿çüÎR
¿ç`oâ*ðUNASNone?ÁQïVŠ'º?³l{^Iy•?¿»ÒóÇ?¹IˆH'ÑI?ç´"IcÙ?ÀÊÀ"9wé?­š_ùÃ<T?°gìçþ?À2?Å!–í?½^Ì|•ý?êÊf€?À"dµÏ+?¿ÜÏ!Ç$?œ@°ÔÕ?À¨\Þ	ƒ?Ÿ·½ëÏh?çõ-cäDº?¥M·Šš?¯…Ó'•…)?"ÜË_£?Ðꢅщd?´T†±g¢Ù?å'Qƒýâü?´2G\hãû4FGL J1953.5+3841?ƒ룝˜ž@¾Ès«ÉÀ9"w3"«À;Á15,2@¾á˜5ìK@žŠdrp`?¿ÈYök®?ĽßwŸI?þEÀi;'@;1KýYˆ¿íª¬çT7?ïô"&"À¿æ¬Žhãï(¿ã¢»a—è¿ëVœ_˜¿Ö1q<-WÒUNASNone3FGL J1953.3+3847?ÝàãIzú?Áµq"6;²?µ•ènjÌô?¯øçs'˜?ܹ¢"¡Ò®?Â
ç"lXÇ?ç£KÖ^¤«?Ƈýc+C?œZ¨`à~?©ÐŸQU?Íç{ši]'?ÅNkv ¯?ãÕ7ã,‰?±|ôÁk?³¸ñÜ£;?˜¸*bõE?ÓgSÁØß_?­9Yjªý?êDÉÛa³? ˆjt¥j¸?°¿Ø™=Í?"Ù"Îòç?½ßOçîœ?—úP憷š4FGL J1954.4-3729¿îQœÞP6À;û¨`ܹªÀ:Æ(¯K²†À<=b†ž@åXvc´…@áhšô­?ÒùYÞÍÒ?Ð
Èâ¬?õð ŽëÁ@±:ªËÆ¿ì Ð?Hl?»Ã!¨FZ­¿âMUô([i¿äy^½zŸ¿ïëÆ!·à¬¿ï"ÝíÜgUNASNone?îgþsÚç?¡ñnÆÓë]?nà!|õË??kP¨Æn"ú?§'pòôÑ?¡NíËã;?ȿ2¢?£.ö~e"?eǏŠªœ‰?xã÷r"¯?£ØŠ{b,?¡ágGp¤e?ìO!ù¡0? ‰Q''MÃ? ç3ÙCù1?PZò€@?µ]#ùå?—ýýtb?ìÒéÎFò?˜e_8q¦?w^+©µ©5?h Uû7 _?·ù=öòmÝ?—¯lVÿpÅ4FGL J1954.5+2420?×:JT3¿ýäH•:À:0S5À;¥Ã<*Rº@Ð3öýwå@L¢À‰Èk?ÓZe¼Tº?äòSÍÝn@à:2*õw@÷l¿›áÈ?ïþ
¡ÿϿ㠝™ÙZ¿ÖÈhûí¿è­µ°P•¿ï÷!ŸŒø¡¿ïë	εÛUNASNone?Ñ2l
0›+?"ûy×è?›ìtäÛÈ?œ4û¾ÙèÄ?æ‡fSƳ‹?ÂïD–VŸ?ÂæN«ÓÄ?¸®!ª¾"W?£÷c—ï"?§LYþ£X?ê@P2ä|?º}è
"å?և׉
Ø?±®&""?ÈTãw`‰?©±è"‹¢?ÝMá…:0ã?±hjžÐ?Ïh>BwÚÃ?ªÎ¿ÖêVP?»#é—ú?£'ªf~?äÁŽ¤ÖP?±ÉvûDæù4FGL J1954.8+2543c?ïÿÒݏ¿ó4(%¸÷À9Q,?#+~À:Ù­´Ù'@
O$«[
@œãÞaIÇ?˧tù|-M?ÖK^£#†@JO‡&ÐN@Õuèºi?ï袠ÿ>?îFâ< š?¿ê¦WþÊ&¿çl1aKõL¿ïñ½m捿á
qs	âØUNASNone1?ֈ˭¨"?é½+Ø;?ÄI­_Ë?½Æ¹)Ul?ßR]¢ær]?Æë»í?±Ü<:è ?±{Ú €ÐÜ?ÏvPÿ[Ë?ÈI¦ë:-G?åæä8Ì'M?ȈM=×ó?Ä2иÿÎD?¢Œ²¼Ÿe?Ç0Vî¾ð?¦Ž)ª!ôÍ?å''¼\³?ª‡ï*?­HeùÎ@?'þ'ÿEøÛ?Ù>‡>¤Ç4?¸DŸküå?áŒ6¸d?·v;^äýx4FGL J1955.3-5032¿ê&&Ý[ݙÀ>'àãF·À:ÀöÞN«À<r¦Q8ø@bü}"€U@ø½=ã^?¹÷(€|½¿·vœ¿há?þ{ÓJ•Oˆ@>•=im¿ãëÙ7>Z¯¿ä[ÇqC9;¿è"ÏöLø׿䦰~ L¿á¬ïícEJ¿ÊNC"å¢UNASNone?ï!];úÁ?š$zb‰h›?a¡Ž¥mA?Z$ˆ©¢ÏC?™ &»_šQ?™?ū׷[?îºlKá?«ßœäôÎ?\ÌK1\º?w:µù
úè?£x¬¡¶ú?ªæYÛÑ2ö?îWӆÒ"?'¶
Â6·d?u`<I/tÄ?f†'¤pˆ?§ÖÀ	¹¨,??ãZS.7?îëL­tš?…Ÿ0båü?`ÜHw…?ê?UA¿!µ? =p¨ba?…bÚñ†-4FGL J1955.8-1657?æÀ-ÛþÀ5¨ßXÀ‹vÀ:i1òÁSÀ;õͧ¾‹@+ÌAaŸ,@\…×Dö?Åy£¯ò÷?OÁ—ËŸak?û€©E5?Û&¸{‡	õ?×wEÜ®S¿éDÔ`?ù¿éhšô¬·¿çÉc‹À"?ᐣñâ0UNASNone?ínÅŽZ…?±¸31óª?yÐ}ÿ^È?œ4ÖXnˆ?²ìЗJ`?°äÅ,
?îë*£™®?£è[!û|ö?s"?ºVt?€ùn?'Yò?¥ËmÏ[?¡Ñ1)—Š0?éWßáDö?«UÄ=ٗØ?š&αÞK.?"ê€?m?Ç[ª?"Á?©dìÙýl?éX§
?¤ÑdÈÆ}®?"ÔåDÕÖ?"kî:?ÈÄã}?¤;Ì­êÆ4FGL J1955.8+1154?ææIˆ_4™À ôuĨ;À;Ž"ÝÀ=óí£*@ "µ$¨?þNÚ"ö¥
?ÛFqÏsÆ?ïn>Â2"þ@߃ê?þ÷öüK@?ÒÖÊ|tW¿ïÿëJw?ïýš)âQ™?Á» <‹v–¿ìÞzt¿ïýSG¥°ÿUNASNone?Õ_ÚQÜXŠ?̶™\ò?°žÄ†X?¬Ï7Ê#&?ã<::Á¿¯?ΦÏPDª•?Ð+"É<$?Ëʹ"˜?Ål¬bÙ?ɎFuÄn4?âVTÉ7?ÎØ΀ݦ?ä83"?ç¨?±'¯aÊ%?½F ïû?¢`ï1d?Ð=ñ·Ä1ê?¬¨ŸiAè?à+jÖX÷?Ä#²¥©?ÕO
%À­å?ƂxixŒ?ĵ€	%@Z?µY¤í6&4FGL J1956.6-7011?¯¦ýo×Ô=À>ç¶þ.n¨À;™÷
ø|À=V%Ýà‡@((ú@@«~žk?ÔÄ_`7Î#?ïÿäâBTä@ÜR¾éµ;@("nmØ?ÓڞF§"¿äëgø6Ýã?âËà=ÂÙ¿àhK_·K¿ïÿd†'V?áécÜHkUNASNone?ä]b°"íª?È®WK¬Y?Ò-Àmž¥£?Çwì?žz?´]èÄÝü%?®k	¹R}'?ÞqÚ9fó!?ÐxOÓ|_Ò?Õ¸08ƒÏW?ЄÝq­¤é?Ç«ë*{?¾Õ±¯"ËE?Ü)~
Ø?¶ÖôO>±"?ÖÖ/œï?¶¤UPä£?Ê÷ƒã?§RCn?Ù֔=u¿‰?ÀIþ¾Âíè?ßçškÐ-M?ÁÐçÐK€?¹EZèL«?¬ËÿûüžJ4FGL J1957.6+1230?ª§£ÂnM[À!_€™"À:ˆ·m¿öûÀ< d©ÍÄD@d'8Ôþ?ÿ'ØÚø	?Ѽ
éÿ
?ÓÄcœ²}Á@ÕÖ¾¾Q@».\^Ñ¿ïß#FV%§?ë[–©û¿ÓN­âü¹ú¿ã¥*&D7g¿âþP§ET¿ïÿýawUNASNone?åä<›S†'?Â`Àíi¢?—!å7?‡
 òbP?ÓJÎhIÊù?°–{?å¹Æ¦Á+?È0Á˜-B?tk.PL²?'oØ¿g.?Ô:Ç$¡<v?Çýð4-Z;?äÞÆ0µ×?¯—±"(—ø?³ÝÏ<_?˜Þ½oeG?сÿۅ9?ªæOR=?êݪTÍ0"?ž$DÜO?Œàü,¸:?wxN§("?»Féÿº?Jû'•í4FGL J1959.3-6121¿éà[®bºœÀ?¦bfýeÀ;¢™=SHÀ<êI"Çȁ@!VH‹´ÿ|?ò+ŽXó·?ã8b1?í'ѹ›—¡@N»Ÿ}ß)@\ƒÐ`«¿ïÿÓõµú"?ï÷AJM+,¿È=a	…:?æ"Ñá^ª/¿âQ'W«¸€¿áÃÙDr UNASNone?ïÄK¢?Œnšî>±©?n§Ð¯«*%?q8+Ý4 4?"šÁOLÓ?‰'ևTaÞ?î'w"꺮?²Ëdº çü?'ISPùv?¡^ºJZ—/?¢"4\€Å?¬®^R£E?ìâÕ¤Öº²?ž¬âë›?òí±'-­?ƒÞάNt'?´¬—léŸ?›Ð°AÆ!h?î¥AҕÏ?™0¹¼‡?kr¿ù?v5mÜj?£õº¡w?˜Œm#8¸4FGL J1959.9-4605?µ¡öûÇÀ>­ú‡;À;ßúTÅT3À<푮éŒ÷@"Y:-ù8?óxÏÞ±Ò?à´/è%ç?Ù¯Üüð¬?÷Ì_‰ÓRù@}%
«:¿îØúØxÒ?ﳬ ›%¿íç^~:˜'?ÉWw¬	?½ y1Å¿áŸê¶ÂŸLUNASNone?ït¡:ví7?ŒµY)T>?]P
Ãû"°?[	כ+®(?-¯©ÅMº?‹F³©Ý­§?ïX fsV`? ÐÌùØ?LÒÓìp?ï?n'ŸøHñ?"\'1±î? &Çq4¥;?íCõM ×L?˜óóc/\?'Ÿ		R?uâÚçÊVÎ?³ŒtuÎóô?—%ºªè?îý§js 7?ˆèûŒÕ±?47ž&¸y?AÕ6¯£Î?Ÿú•Ó#^O?i'Z…'?4FGL J1959.9+1833?çû›[)‹À¼Pbîâ¡À:|³_=}9À;ç¶jŠ¸U@æ"Ôei@™íeÊ?ÏMò?Ò³×Ùõ@Ëi¥¶Ž?û•P9(j­?ïýà€ˆÑu¿æG¡Ÿw¿á·T*#¿ù¿àÑNÂò®¿ïýZØ®¿ïýl<i<ÚUNASNone?å"t—H¼?ÂÑù 'Ý?¥s@'ô{?³H¦€ž~?ÓHg.Ìoú?Áaíhð=ü?Ñ- t`ª?ÃìAƒ#&?ŸöžÝÕґ?¥ë¶ÙiòQ?æiĸ×!?ĜBÌBð*?àRZ¹@†›?¯ÌØåhOm?ÁÄ*¡ú¢?¡nÕ(-?Öy5‹-õy?«<>È}«?ÙFÔtú?ª5[ûíBP?½½»ã)8N?¢VaÇÇ?ßI¼íÀ·\?­w9ÓVÁ±4FGL J2001.5+1611?ÝôÍO‡/gÀñ¾±ìÀ:ÞkZÁíÀ;Շºtµ@ý-Ûö@Æw}åÞí?ÐR—\R'G?ÛS%âØp@(Ëwb?ùqoXþHñ?ãwÁm9Í¿ààM³9ä¿é	(Ó]à†¿ènn¨TG€¿è±òá‰rZ¿ïÿô╋îUNASNone?ÙITÝæo=?Ô[¯ð#?¹×²,aY:?²ÄX£÷ôu?à _K€9?ÃÔ°ºòŸe?ÓL'm‹?È©zS÷É/?ºKéÓ03?º…Iþ®5?ã5\…9ã3?Ë]JH5nÍ?܀!Ôºà?°3¿À—²?Á¥Y$? ¹Ö@"@?Ú­[àþÁ?¯6úÅ2&?Øv¿î[Åf?§Ø€å'?Ì̞Eú‰i?ªY=‡¦?Ù"ðî¦õä?ª5LXWn4FGL J2001.5-0958?íñ|1ÝP[À4ß«÷jÀ:•GûATÀ<ÝË!Ñâ@QaÒ-ø@â
Üa•F?Ó'½ÝEÁ?ÃU´'Œ¶?òÖ0=µm5?ù(ï7…Ó?ïšúAп睨ÇßÓ¿ëý7Þ¾'Ì¿åÚKäÚá¿ëY*GÒ'?Î}šàkUNASNone?ëw8úÖB?·eWÛ= I?'y>¢ÿ? è8ø•ƒ?¾¶¨€Ëõ?µ}Z†+ý?í=ÍA–"?³@[óf?—.§*Ë¸?¢Z¡0.MQ?±¢gË@ˆ7?«E!îíT?éÚÇßXÇ:?¨µè†ðâ?¢û'Ñ?Žaíð
y?Äa¿›Âb?¥Z|F©¢?èÖäOs3ã?¦öKMÎ?¨e
9R¹å?–97ú‰2?Ƌ,3ށø?£ˆÒ›'4FGL J2005.8+3357¿Ù«;/ßtM?ñxE܃#6À9VÆÀCQŽÀ:›tkâ§*@ >vx'GÃ@ãÕº²?ÁYɟñ¢o¿¨-;¼2Ž?ð%ôkwG_@ö§uzU‡¿î
9	6	§?ïí֝0'¿çÕ¹€ቿë9ÝaD"ƒ¿èïî:ß?Ŕrþ¥7UNASNone?Ô!Þ&«"ª?ÒXu'-?•¿F¯ó?˜ƒÝÄ
Á?åFRòt¶?Ä!ký&NÑ?ԏ‹üú"?ËTÙð¡?b²x,&¸?¡x‹ë-?åx¢¦@!?ËJiO?ÖÓ®'Ӏ5?²·…·˜Õ?²®Ÿ'E¡?&XKÚ?â@UÃ÷1?²iظ3?Ї/'µ-?²ìIœÐh]?"²¾¦'?zM@ÏsÄ?çi‡Õ?³N3Í[4FGL J2006.0-6538¿êôôx"ÃkÀ@ï$©ÁÀ<©1½nÀ=¬tg°é@#'ó‡÷†?÷%ˆ»%œ?â}Ÿ"Ò?Êb¯ã Ü?îÓ·¢™œ?ô qÇîk®¿ïZu%F¿ïö†5•8?ð¿Ó½SG¥°ÿ¿åËJÍǟ?Ðmû½ñhUNASNone?ï3.û5?Š˜»Ó¾Š?>~£†?AsÞy˜¯?‹?Cœ)…?Š5eÞi?î@ð°ì;?²Ê><–på?t4¡Z¦Æ'?‡N¡s5?­u\ɜcu?±©¡ïO?íeø5ÛóÚ?—ó2Œüõì?{Á~ßT¦?vA¯–ôwµ?³ò92kâ?–ìY"Ôo«?ç=;bØG?¸å×>Ñ \?b0ðù˜?j†Óà‡´å?Ña"Ú)Ð?¸êª@hŽH4FGL J2006.4-0354?íb‡×­ÚÀ2v…¹èÄzÀ:àUӌÚÀ<'ÅÅqŽ¹@›,™f
@a
;Ã$­?ÉyD$>û?•P?J£?ÏôÔ¾2Ö@þv·Au@?¤–á?æ°§2È¿é¬"qÌ¿æq²à<–3¿ÄïXgö…¿ïóqal+¢UNASNone?î ³bgY?Ÿ
?n뒮&ª¢?pʙÇäÞ?¤®«ß¼?ž$B©Q?ï…$óV?eÀ_§?D=w½›Ÿ?\Œ¸·zY_?zßG^p¤?‹ùé<²Å¹?ì=	=1/´?¡+Ç}3/?Šk\ÿ©Ìì?yŸ±eZ˜!?ºÊJvHÆ?Ÿc$RÃà?î?Ù^El€?'õ¯ßjí~?g ²nÜõJ?a:^]Kíy?ª^ô»h·?'†Z²Ó&4FGL J2006.4+1834¿'ñ6!œÀýۘAªÅÀ;'~B%>À<Xæk"@ òc'?ýlÖÂïÔ?Öô¢Ô«¾_?Êö²¤W±?ùŽ"î9.@–Ѿ#<¿à O–@I?ïñQçS`пíî+÷Տ?ã_ïSàR¿äËôï#¿ç×Fm¢šÊUNASNone?è÷ìHÚ?ÀkÝè&?vDӏ²ŸM?‰` Ç|"X?Ëqi²_Ë?ÀM^ãç±?é:©S€d?É
Ä®¤yÀ?Sù
\gá!?q­Ã?5WÉ?ËÃ#Eù.ª?Èå[X€f5?éÛþFŸEä?¥†È´ÿ4X?ŠÖ‹lƒÖ?wÆAÐ%×?Æâž.º«
?¤NAÌÈ?î®Ê%Ú[?•[ß²†mß?mß
CNJ?r+µ›ïiª?£@¹puh?"‰@ʟ~4FGL J2007.0+0707¿Ü?N ˆ1yÀ*"œ
!¼À:2wKøÀ;ðK+w}@`Õ²yc@YOýnUH?ÉÃ]wÕN§?®¿»ŸÜ\j?å:áqÊ@҉SP_¿å$ô,¿æ6¢ôŒ.w¿äþö€$}Ž¿çiqÛ¯¿àîç©Çå¿ïÿóÖ&ãUNASNone?îšù
ú#¿?¥ÍËە?qEIP"³?gc…>W'K?¤'Æ,³¿¯?¥v·Dˆ»Â?îT–¾»Óé?®Â$¾=mN?g{&jõF?y
]—,€à?©>᭓lü?®
Ywî)å?êjЮFÈï?§ë‰É¹Á?•úÜbÈ?€ükəª?Õaº‹Ø¦?¦ã_ë†?éÏÝ_AÁ?£¢K}ÑWW?wEû?hO—­£ÿH?È S úè?£ƒ0PŠ…
4FGL J2007.2-3157¿ï:Ô.ëÐÉÀ=1ðÃLÀ:=ƒá¡pÀ<<Ãþ¬C@+,õVƒÅ@¡|å-ì¢?Äaºö¶€?È´ÃÁ‹P+@¨³Ûd?E?ïuo]þ/?îגŽ¿Â4]ë¿ÝôÑc4'¿¿âŸ……`ý¿é¤IöÄ¿ïâòÞ¯M`UNASNone?éí◾ç1?»Y‹Ö²~V?¥hF™U6?¡â1¿f]?Âîcú¯»?¹#\ì¦p?ãuVºó
?ÌaR4'Û?Ƚî§GŸ1?Çs:KQ?õ?Él¶lìX˜?À3©i©,	?êˆF×Àæ¬?¥qo^{â?§è;Qu?•JÐx¾%?À*'6ð?Ÿ'Á-œFP?ÒË·Jicø?¨€7)2ì?ј÷'D?®ì‡Q^»?Ü°¦ŸÄ?¯"¯+dj4FGL J2007.9+2511?ÛÙÁ¹PøÀÌ W"ýÀ:Vã®À;Úà!p"@ŒÛâêE"@Â&ޑo?Ëk›¦ÿ?áqðþZcy@•ÚÈ8?ìÙAéj£s?ïÿs}¦¿Ñ¥!øxLB¿š…}`††¿ä'á4¸Ä¿ë=3g5™?¿ëëԚ ¨UNASNone?­÷'xï›t?ÁÚ>:?аÙ1àN?Æfot1?åÈ?#?ɧ > ?²9˜#zlš?µ-öå]=R?Èô˜~*2?È/89åÁÊ?ç{¦Ü	§à?Ç1o镇ñ?Ïw'Q
[é?¦ñá—Øû¹?Ó/biçáš?°è´
¸ò¢?Ý	í'pq?°?'ìüð?'"-ïCÓ?u'[=úèW?äaV½ì-?¶"ÐßR:?Ö$e3g?¶+ýùt4FGL J2008.4+1619?ïÛð3â¹&À!§"š|©À:ÐI!²oÀ<Aٌίü@ {3§ø,?Ñô{<ŒMV?âÛ ö¼Š?ïÝÊì!üª?ûº£º"ˬ@¨[#*¿Ý]pH'¿ì9)í9Sß¿æîá(úJ?µîÓTPd¿áÆsxŠ¿ïÿþøþ"UNASNone?çèGŽå!?ÆCg ¶B%?|Âó£ÍZ?hâuHA?ÏxÅ°WM?Åÿòò¿ªL?å"Ñ#Zñ?ÐI.|©ß?o9َ.62?.1lÉr?ÕÀbªœí²?Ðu¤†Š?çàØ]\ž ?¬'û©£.×?£6¼™³?õT@ôÒ,?˘ÛgÁ?©õ'»{Ç?ëü¾J§à?¸­•n·?8'7v¬?PèNÿþ¶Y?ÀŒrDÁ?¸°øP'O‡4FGL J2009.5+2425?é1«òjHÒÀïdþ‡YüÀ:Šh¤.HÀ;hFDe@cÉÑÅ°@§ÛðuI?Òò)=;å?ÜA^#÷«ô@äàTi
á?Üϧº'i?ïþr–öQ+¿×æÓs¯û¿ç=¥b$¸F¿ìŽpK™\¿ïÿ']<9¿í·ØIёUNASNone	?â#GDËx¸?Ëè'ŒÍk?³{´L¹—y?ºGm˜[?Öڄc:¨²?ʝnwv?ºyOx-¢¶?Áø3ˆJc?ÐQ˜Qì ?Î'±0Í׍?äˆ	èl՚?͗"Öµ¯?Ìô d;d?¨ˆV>4ã´?ÃóHQS½q?¢C,цÄç?ãÆҋAË?­°H@J=î?"›l¾Ôˆ;?l
¸œ'½S?âÏØ(ü?¹îiÕ¬??Ù»tg·b ?¹'›¤¶ái4FGL J2009.9-2116¿é#
"1œõÀ:ZA€ÓÏöÀ;	±oy4ŸÀ<ÎÛÈRé@àµFsW?ý…Á•a&?ÎMúI\ÀJ?ãÃBàO`@´Õ½6VÔ?üæÒâ¿ï'¡­º8?ïþo§WÈ>?Õ-•d€³¿ãb:[€Y¿êÇ
H½ß¿ïÿ²2ӁUNASNone3FGL J2010.0-2120?ßqü
ÅÁO?Åz¦E)?Ú×!Œ«>:?ÆÇë%˜Þˆ?¶Û‰¢<Ù?°&ëÁ,Í?ÞQïc)¦?Ê Fá1?Õ¢‰à
Eý?ʞى€?È
y˜'?¹¹0‰–(è?×Û7–?¸:qjHã?ݨ™~ø{¸?¹ÂQˈ?Äø "܏?¥‰U¹=¤³?Þ!LšÌ®?µ…³÷\Œ?Ôrµ¥ž×0?¸ÇZ6Ä>Z?Ê×ü›Œ¸F?­LEtg34FGL J2012.1-5234?í£Þjð À@£}é9êÝÀ;CšMô€À<¢È£r`p@"¨YßDs¢?üé
	Ó¾Y?¸éú=|b¿ÀJNØ«'a@ñÿ ÜïZ?òà-"ã§Z¿êiU./¾4¿ãºßr#¿ìyÄaÄ@6?ÞpØûYR,¿é,Žž"Ô^?Ð;e[Ï_UNASNone?ïw¾ÜEB?¤#Xx]|?OÓ«åÅÑ»?lÊՂûÒ?jÅI))?£ÕOì|bÎ?ìùð}èì?À
`Ѩ§®?™TOcž{?²|#Lä?±Ûh0_¸6?µ§Û×"‰Ï?íÝ4¿H?žlƌ?;³?{W9"Ž?x6¿%ß~?¶/@è"D‰?±ãŠ7?咓#r"®?¿´£?÷q¯?ª-݄›š?ª¢°¿úYu?ч3ýjE1?¾Jˆ½SNw4FGL J2013.9-8717¿ÞS6'}	…À<°_®¼À;¤'[rÏÀ<֑¹ÑG†@!29OWB?÷4Œê^®?Ù=œ˜§?Ø}jŽê/?þw'Þ"um?úàï""n¿ïýxÑ¢õc¿ÝñïÜqZ‹?ì÷ª%Øם?²<£Ip·M¿×6‹{U6¿èŽá¯²áUNASNone?îô½aRú?˜AçhgH?W©ËT2?T[Dߟ@Ñ?Ÿí¿šÐX ?—ÇÒÖä?îþ°·ïc?•íŸÚl ?[Ã;QÊõ?lvõ˹v9?žxÜÎhÖî?œ
nKÔc?ìúE'hCÕ?œW_€çX?ŠQ摔Ï?MŠ¦|µ?´Ûé/뮼?™N".ò5Ñ?ípìT£â? W…$;Z?Uå½ùó‰?RêÕ?ğ?´!búï»? W-9Ñ34FGL J2014.9+1225¿ë»rkúœ`À(n$ÛÀ:¬%¦'¶(À<rÛ¿®×@'}‹qÞ@|Zœ-Ȑ?É¥>}êª?¨ÙMþTs?àá¡Au@Uzæ{¯¿îxx¢(3{?³/ÈðtFÏ¿ë[iw'ß¿Ï*ö´Ò°¿ãê–vÏj6¿ðUNASNone?ï#²Vª¥?£åOo"‹?išâŽÍ@–?ufjØ=•S?˜V`ãQP?£oÝùámÊ?ïBÍõeT?©§*'LY¯?Cà0òª¦?V]7h"n?ŸX¤À›À7?©…cj?3Y?ëSڞG°?¦%iûÕW?'ª.Ç•ˆ?f;:l¹M?À[O®ŒÞ?¤eÞÛj'?î";Âá'Ä?'…áVQÊÈ?nðKž:ì(?`S‰êù?«í?5?'	ÎxC0;4FGL J2015.3+0758?ïmœQÀ-:}ªOÊCÀ:hꭈcçÀ;ÙRé±ßá@…xÐK\u@üô}þ•?¿å[9ºH¿²Ûae¿c?ów¨Èá…Á?ü³…ü-ãh?éà"¾ŽE©¿êûêâa‰ˆ¿å2d×.¿ê÷Ü_ïT¿ïò³±rÔ3?ïҌ)nŽSUNASNone?îÙ¤û?§dÃ×:±?m=—
¹3?kø±ùß
? 'äí§Dq?¦¯®›—E"?íÊ¿ïÕ
?²¾Z?"L-–sAy?'ΈX¸ã?®@õ]¿?°žƒ…
È?é¹¼<@'ò?©ÿ®"Z°ó?¢žîãK/??Éo½—?ÄqSV8¡m?¦ô{:üš?çñ°bëM:?±6Ø!º$'?™»3#HP?Œîe»!£?ÍØéÇ.?°Sï~ÃUO4FGL J2017.3+3525¿Ê&ÈÅðÔX¿´u"–ØÊÀ:Ç>A".ÎÀ<)I`œ"@!½Hö>
?ò_æ¤ì´?Øu\"•¬?ïÿïÚê@
É?äò]€?ü(^Η}5¿ëÖ?rÖÚ¿ì| ·Ûy¿Ò]
øGv?Ëz£_@,k¿åê{3}¿ïÿ~?ËòÝUNASNone?ß®PÙ?È'×q‰?¬H^jcý?©'ÜU#Ü?ÜÈèß¼™¨?ÇÂÿ!Øk?¼*·k×Çå?Á¿n‰Ž'!?±ž¹?¿=ªë?êFå›U$'?Æk†I+zR?ãVÀ
Ž;Ê?°Xb,pp?º'ÃÒ¯NÔ?¢dšçŠáÞ?Ò±Îð7´¶?¬˜š²QÔ)?̐½Å6‡j?·ÑÐ'í&?´í!‹¡?´?$]{ôÓ?æYÒìÎ,±?ÀRí±	a4FGL J2017.9-0114¿Ø#8¡(¦ŠÀ3¼î9.÷À;öÜjςÀ<[ƒ°úo@ræ@fU@
%ó¯?ÓsŽ!ì8ù?àèS¦pA±@ÚcÞÌ©'@§æž!ê¿ë>L×I''?î‡óÿÁ–¹¿×ó{B¤,¿èš† @¿ïüð§12¿ðUNASNone?íÿ²VðªÃ?©Ð€¦Ëº?«ä'*e?¨)æ1L?ƒ¿ÚA¥ï?\"–÷Ès?ç`PùС?ÅK>²tÝ?ÂyÚ:n:?Áåpwö3"?ÀáÞQvò?´Ï˜·¤]á?æ¹ïdzô?¯L1É¥?¿ÁÂYs/`?¢0Ëÿ¨Gr?Å7b¹´|}?¦¬ÿ^")?à+7E­Ø?°õ҄jÅ/?γ*
ªÝ?°îäÁ_ ë?ÐOüoOAã?³Qtà‡Ð4FGL J2018.0+7903?׏ݠ&@6©˜áõ²À;É+ml%À=Kh;R¼e@þµFÉ= @lñ<îØ?Õ×Ä3êé?ï&p­F@P¨>x
Ô@p£V0ä?Ô_2€ó¿×dŸg™¿¯Ó.±Í¿èélÀ"{¿ïÿàöO}¿ïþ€Ǒ$UNASNone?åؾ}Š.°?È1§nÑ9?ÈH:9?Ácí¸zÆ?ÀŽ½y'?Â\ÂÓ@	?Ùø|c˜¹Œ?Ñ	–Í'¶?ÝcÓ W?ÒÄK†ïƒ|?ÁÜ?'›L7?¶k'ìÛlÂ?ãÇ—ò?±;	†:?ÈÉ ö_?«F?²Ê£?È,­*º?¤ôiIp¿?Ðv¦Ÿéºh?²e.c㻣?äÓ&`®f?¶wðôÎk ?·Œ2zåæH?ª:hIÂ.n4FGL J2019.6+0616?ÙݎbÑ'óÀ0cÛ]‰HÀ:žcʪ³À;Ûxâií@ã`"jZ½@8ââ¸Ç\?η:ë
€?¿@1ôCß?óµý˜F³C@Ún9™~¿^£úF?ïõŸI[ê¿æ"@ ×f¿ê}ó¶E¡Ë¿æª§=Ç
ì¿Ê£]½ _UNASNone?퉌ž·OÖ?¬%Ï_&||?"KºÒLÀe?€¹›yEÔ;?±*#¯ûéG?ª÷ôJz¨?îRdâ=,A?¨™Iœ‰×a?{ڟ!š?‡'vmZ?§xöˆI³?¥©ßãJ<ó?è¨8à°?¬Ü3+X?œ²0fè¨W?†Qã;­m?ÉÈÖrà*«?ª¯Ò½Ôd?è5aSFø?§ë7Ã`¶?"ÊQ"7²}?…£†S6?̱1¶+íÓ?§Ò†åýA4FGL J2021.9+3609?éʎaµ°¿Û5L½j¯À;hÙÞ-GÀ<
Ž7eÇÛ@$‰ç˜ã?éà§_ªài?âÛþCx?ïÿH è@uúX S?üJÓlN2¿ïûš?±Æ·?îJùÞ}Ï9¿ÕÒ½<64¿ïú²]à°Ú?ïåe¶™…?Âw´ÂiòbUNASNone?ß*†Fúu?Îôó¤s
?fHÈ ;?'ëÏ~ºÙZ?ßώU,ƒ‡?Î߅9'>?°«þ#ä%7?¹µÈÂ
‹?–:>Wÿ*‡?­s%v÷9?í8®HÂ?¼ Â‰ñ¢?ã,Í^àÐ?®'/*Kß?µç±J‰?›¾´Ž59í?Ô, ÕúT?¬#V{\šÇ?Âö•d¥H}?»ýái?yhț|'?''g©ó?ë#ÕEvç?¼["*)4FGL J2023.3-1947?áè€X;;§À<ÅAÈ!laÀ:Gû'½À<:»9&';@YžP7¥ß@óõÞ>Y?ÅI©Äå?Ä1s*.$?ûL¹ìö8?üþS¶‹¿ÜÅ3ü0耿åóû_‡O¿æ"f"?=¿ç>¸Ø#B$¿ïÿ*LÚ¤&¿êá'V¯UNASNone?ík§!¶?¬+
V"ö?"¹lÃN¬?'C@ô†o?¯hØLGŽH?©Ud,e<?ìÖ.ÊÆ?´Ð'TEÃ:?—äŽ7 ?7y¶%|ï?ºø*ûèË?±Ûµ"óS?ìkðhw? Áì=e:(?™Ød¼ÏŽ?ˆkÔý.çJ?¸ÎŽ1HØÅ?›t–¢ÁÇ|?ꜧø1º:?¢=4†,Å?«+[©'ç?"öEÌþ	™?½…i©ž¼?œÛú¨¿;½4FGL J2024.2+3616?î¦Ánä~¿ç¿û}º@À9¼L¼ƒ©À:ÊèïBB›@ ¸dÁÅ@XÕ[ç‡c?Ð5†?º•òpw¿?ï¨E™gD³@
,€ÛÞ¿ïù}Ðwl?ïþR€ÖT5¿âß̃ѱ8¿ãV¶Zš€I¿éÆyÌt¸9¿àEa3 ¿UNASNone?Î/ž˜ãmÈ?¿\"ÝXb?±X¼¸Ú;?°×?å7?æIÂÅIF?²Ѡ§ Q?Ä$ëƒS@ò?Á™®
4?•â=þÏb?ª{×¹¢b?êG³/:ÑI?Á|æÒ@n¦?Ë?pN%?¨ð'uþ!?¸\&cé‰?Ÿ¨ûƒÌQ?æ$¹êWoF?«}¦Ç,Ö¡?Ít­ÝFF?«Ê¡Ux©?™f¡É ýÃ?T½¤n?çןzat€?­(¸
Gô4FGL J2026.0+4718¿ì8H^¯Û@^ÂRˆÀ:Ót«£‡YÀ<n´Ý¾V@ø²m¥õÈ?ÿ-5Ã0kÙ?Ӄ_èÈ×?æZË]a'@WgZ',–@²³HÂ;¤¿ïÿÒH6Ðw?ïìrº1¿–¿¥äká
؇¿ÒHSUèiá¿î1"áHÚº¿ïÕFƒrèUNASNone3FGL J2026.4+4709?ÖüI/¶UÑ?øG¬'Ð?ÊÈÌyp(?»l'pUÑõ?ÛûÒjò?ÅÁ¡¡LDA?ʧÏø?Åhce)—N?Ó=ï%.*®?ÊÎ+Wf?ßn(ÞZ
‹?ÊÒ à1,?Ⓔ¦¨¢?±Af…ÐÛ?Ä	F¨¨…&?¦¶¶5}?ÐÕç^[´,?¬¤×ÅF?ߣk@üÒp?´:ÄϬT?ÑÕʔä¿û?µ2¬/}'?Í
"T<Û,?¬¿ô;?È4FGL J2026.3+1431?çö|'fŽÀ*ãjËGÀ:ËSïk]FÀ<«[ï@ôÙ4ª,?ú•çéóN?Ïȅ?o'?â=>»&²@‰`ÈW?þ§^3$k¿ï쾤ëÝ3?ï{ÆKç_¿·¾t¶¿×»o! ä'¿ëko"óh¿ïþÉA‰UNASNone3FGL J2026.3+1430?âRF#Gú?ÆÑ=.ßã?Ù8¨+…SH?Ç ¾¤ÖO?¥µšA æ#?žtïå"Yÿ?áˆùçœÍ‡?Ï3w	³ðß?ԐN÷*Z?ÍÚ½§öþ?Áª÷Þu/?º~Lsî?ÔL•Iy,?¶
îBP[_?á,8ûÀÁº?·ûšØ@Ó[?µñôj¿?¢êâ"Ék±?ä/±ÁE/1?¯'`sÚ¡?Ênÿ±ù˜«?®dX"˜—?ÄÒ9Hñª?¢Á4D±[@4FGL J2027.0+2811?ÈÏ<>À‡oó­â&À9¬ŠS«x¿À<©"àß@Ans{!ß@z*ž9;‹?Á *†<ð?ë7ZU¶ì@!ýAØèd@YøŠ•Æ?ïû/²?¶Âa C?¿Ü7e\{+¿íô×x!yÍ¿ï÷M@ÝÁ¿ïÎ߁Z]šUNASNone3FGL J2026.8+2813?ÅINð'Ã?Å\/öaœ?æÕ
ů?ɗ‰ÊÀ¬?¾Äû—ò3˜?¼Ér§Ë²?á†?"Ú{ú!ày?éæÞ§ÅôJ?Áü®Éò\?ƒ"ÂÏÎ?ÁVd礴?¿¯Ø fÜv?¨ú"Ú*?瑆Ø|
T?°µÃCM¼?ÁáøMÜhu?¤gbýÎ&?€|>VWN?l™ X›»é?íþfT–Ã?eß~á•Ê?«ú‹!@O?›ªس_¯4FGL J2029.1-3050?îìÜ`yÏÀ@­
A1"¸À:¬\qðÞ$À<6.#)@"Pðˆi@P9Ô7$?Ñ9¾½•wK?ÊûW2'?õ¬8Ï
@öåS+v%¿¸K"@'ý¿æâCÏb©¿éÍÕáH"Ô¿ätáÙú2¿ïÿŠ#ÚМ?¦¡€Ã´ËUNASNone?ï§8Òih?}´ÃR6ö?kXhrK?fß3öÔ?~·—t¶?x@& -Þ/?Ž:é	?£—'!¹s?jþÅöPj3?{àR]Õâ?£d¼ìhË?¡µNÄg0w?ìíÜ*7/?›RêIÂR<?•6³Í2¶?…™H`>Žï?³IÙ±ºùÓ?•"±Œy·õ?îüŠPS!y?…-.Iؑ6?lu"Ý·?YðÚå}'?œà1[µG?"ý¸î–ý4FGL J2029.4+1013¿ë9ãóÒBÀ0dô¥Xê}À:Œ^×ü«¸À;ï&<ª«:@÷\1X$@Ìa¢—o?Ý$‡¾û¨Ø?ÛjŸ(Ï­?òÓ<7¾³/?ø"ãäës·ˆ¿ê"k'Qտᡚÿöø¿èLewS¿ïúý—oó®?ï€Ú…óUNASNone3FGL J2028.7+1012?è¡z/†‹?Án¹VK¥?"Ÿ²¶UÙ?ˆº©Z?Ì1–ë܈??Ác8'jÔV?í(þïeêŠ?·š‰¹GxO?zV,žr¶?žÌ7†v0?²™rù©þ?´ŒÌëô'ý?äÿÿºm²È?®Hÿ!2?»1ŸP? }ÇX"p¢?Îg@F¿ŒÛ?¨7E­"?å7<Ó´…?»úÞïÍé?~íœ"?x×BÂðÃ?ÕV¥h&"?»áà6¸Ž4FGL J2029.5-4237?ïÞºæ,ÀA¾#ˆÀ:͗ZBÀ=Ð&¡@Ö	³2@®ü*ˆj?ɼÿdύq?ïÿça"¯­@ìYÙ?üŒUc_?ïâTžgߍ?ÏkY?aj¿á矶êy¿ïý6AZ"I¿éނ¬Ã¿íœݰʹUNASNone3FGL J2029.5-4232?ÕNGEe,?ÍיÞً?ã'únhA?ÏV²¸` ?­_nÜþR‹?­'3K2?­(Ä&sµ?µBG¸?ëg¦ðÿ°?Á<ÊÒN_Š?¶2°µhȦ?´Ú´R?Ðë®Öª«–?°§D¶Ÿ?á—zFÁ¥]?³÷Up¥¢?Çʹ7¤]?¨ÓeòzMÊ?‡»äºƒUç?;•%uÔ?îëüꬻD?—ÀÌÉañ?–¢pM&ì¥?'9E†O±x4FGL J2030.3-5038¿î?N\ââ–ÀB% …²À;MäSÒÀ<¾ßê¶ÂŸ@!üщÊï}?ú¶_¢ýÆj?È¢{1úy?«s¤i¡?ãè‹9"†@ñðÅûLg¿ïøª*s?ïý`t#"¿Ê;-½þR׿³½Øþ‰]a¿×(¹|ãÖT¿ÝáÉÿ={UNASNone?ïÜÖtÙà?g"¿2õ¥@?+»g2Ôì«?AÐËH·Ž?p¶êYÞèo?fHzòÜÛt?ïš=Æèî?‰ŠV»Õ–?09ì$Ve;?DÕД	×?ˆî¾ä¡­/?ˆÿ™½™Ì?îà¥À»y?øIþT^ý?jû·'`	?Z±RlA‰¯?¬¢:3Ë"n?OQ·d³?îõE¯5‹Í?"´±pøþ2?U3tn17d?IªÎæ	6;? 	i5¹n?"'Ã9ρ4FGL J2030.5+2235¿Ð;³À#yí9SÞ¤À;8
‡=À<'JŸ`ƒ@!‡'Kœ‹'?ð7`Sý®?àXBaNz?îLYµ@˜Ôw¼@.¶YBç[?ên^ýçKÿ¿ïñÊþ@9?ïþ
a'l)?pu¨ßÄ¿á'ïXèϿⓢt3®ƒUNASNone?ã´
Ô½œ?ÉpáÂo"Ñ?‰R$+Dó?…èJº?×ÍS5*¦ö?ÉMéÙIu?܎6éÎ
?Î0‡þT¨6?‹Çˆ@ьž?¢_eão?áIÛÇÒÉ?͸Â	ÈÇ?è¡ÙÉ7F?­Nvðê›_?œ>ãG™Ë?‡q÷ÊÆèz?Éð¿€2/®?«eز""?æÈñÿe…ú?ºçJ|3Ö¸?|ç¶;L?}DÍT+4?Ñú¬Ò?»A]1þ‹4FGL J2032.9-0005?ÞÈ"Îå'À6tÅÉ£MÀ;nãª2À<f©¢%YV@ºãÓNœ@{GA1M?Ĉ\ÛMC¿£¦8ŽfàŠ?ã\g	#•?øÃÆ0{s?ïû<aZ8¿è»¸¨Rš¿ç!Ë+âÜÚ¿àÏπÜ3r¿å¦v î?¸¦g¢0UNASNone?îÕî.¶W?—Ítüy¡}?S•k©­j?M"Ûô?¢q·QqÍ?—z`ü®D?î~!¨Eõ?§UÖ?q¦/ÃaC¨?'ZSC7Ÿ?¥é…Ïx7?¤ú‡+˜Å?톚†úL?•×ÇÞ4?wleþë¬?dg'êË#­?²Thú8>â?"ÂU¦w³œ?éR³ÇYz?§9a7å;?·H'("ž?~J|ïUü?Éó@§ÐÏ?¦Ñõm<¿¨4FGL J2035.3+0557?èŠÚöŸóÀÀ3ãêòQÂÀ:Ê°'Úb¸À<#à{Ö:@T­›"*r@͏ãÖÕ?ÄT±2<".¿ªÐû«©?äíò¼@®)Zvå¿ß²køvžÃ¿æ°ÕÀ'U'¿ïÿþˆ0»Š?ïÿÃÏÎ	
¿âgÿyÈC¿ðUNASNone?ïº"{®f?¤SQ³š·?rLOg‡¬?£¸î`¨{?pà"rÁDî?{s€G*?ïÔ2ºç_¤?'beŸ¶°?1ܺl7"
?Y'ÜÂ÷x'?tÈÖ医–?P:BVO_?í[ƒÉNbÑ?žb¤BS/!?të­-‰ ?iÿ«:Œ?³Õ&â¼ÐÜ?"‰n*""?ïÞòÔß?q8vy'Ò?Bõ¶šÄº?Y¼ÿó§‹Ú?m*Ÿ"oÃD?o¢LÑ¡(4FGL J2035.3+0354?Ù\ég.¯¸À4÷Äâó¿À:éʄ0'À<Ii¦ŒÇ@âÝ¿
qƒ@(ˆÝ‰³s?Ç˂õ¾2«?™3èòŒ$?Ó5`F²?ýwVô-ŽÙ?ïúÏtFùº¿èΞÃO ¿ç§PÑÑ¿æI´´¨Ù¿ïÿæՌŽï?ïÿ˜ÁØRUNASNone?ïFÔÜàIì?'h2©'?]B/$¯p!?W\4òcE?•QAq«Ë"?'ð
=ºZ8?î"ùÈ+Ñ?¥`¦0ü¡ä?tÄ°¼i|?…Pßþ'?¥Íe³f?¢­55Þ:É?íp;OӁ?•,²ÔC?‡Û&%HA`?xÿ¸«?±'À¼ºïm?'–÷+{?ëÀd«]î3?¡~"êS
Ù?‰(<mÔ×û?yçÓ0"?¾×ÓUóf? £¸	n´4FGL J2036.2-0207?í>LõY¼À8/KøüրÀ:¿­FÈBÀ<dLÒJ»@}Š?©r@ï !·"?Ðx $Î?Ù{Tà2@Z&–m@Ý­)ï<¹¿ï§Ù}µ7…?ïÿáÍì¿à©ß'1.¿çôïËÕV¿ïÿõž}.)?ïÿxÃÐ¥UNASNone?îIòßØ×?¢Åü;­ŸÍ?ž'ö27?›ó)©0¶õ?˜¶¨'²ø?"ƒ–&?êpn¾kùÁ?¾À×êi?°¸‰Kئ?´FYÐø+³?»ÄûTYU?²:®+ß%E?æßØ; wl?®"§`08ß?»‰¹àˆâ9?Ÿ@ǐ±Û?Æ»Â!9±4?§F4u(ÕÌ?é­ùs—?¨×ˆøº'•?´FcÂ?¡\"ÆPiÏ?¾P«¾([5?¢ò
'ÉÝø4FGL J2036.3+5642c?Ó«Æ2åì•@#Lµ»8PÀ:T˜ÜÛ7ÊÀ;ã·½q7@‹«(7V®@JNz·VC?О¿#@ø?ՈE^XûÅ@osۙï*@,ªžP8?ïÿøãú¿ÝòÅÅF››¿è6ÝâžÆ¿é@€Þ·°Ü¿ïGY•?å@\FQóéUNASNone ?Íî2ŒL:?±vAzÒ?¨þW²!F?š›4Þ|'?ç—7@Ÿ[ç?Þåx)@Ë?áh3XUµ#?Ìù¸þb?·a%óÖT?·
§I{Q"?×WOÒ_›?ÊÖÐùj-?ÞÅ×Ì›â?°>	KB?Ã<"÷ä¤?¡Ž/^ˆl"?כå·KcÌ?­ç{‰?á•Ò#?®çÀEûw?·%¨=•÷?žLT»ë6®?×[Àj=?¬s±¿F»"4FGL J2037.0-2826¿ïܽ&!ãçÀA3»¾‡¬À9âÓì{¾½À<@xã@¬˜@ßÿÆÜH@âE¿ý±q?»«É᤹ø?½ÌR֑?þ˜ªX-¾@%ô†O:¿ÙlÿiK¿äsãýjúJ¿æay,;È-¿ëeØÂ#{…¿ãÈ:@¿ïÿCÂw‰NUNASNone3FGL J2036.8-2830?ïÙõ›¸—?v	'ž6ìc?9‰ô¬4º¨?5e'±ö?ql'Øñ)d?uv['Å$?ï(Ó±Th?Ÿ'í*mýR?R‡Z};?g|8o9ø?™Öè}ŸO?žql;H	R?ïE´¤R?ƒ¥U«îƒ?l­ëÖGy?fÊ'´r¦?˜Á§bP¬Î?'#™"{šw?ïLËHnØç?{TED'Æ?h‰Ò¥q¬?Wµ-ߛ¾?"Ut7Ð4Ç?yá:xŒ4FGL J2038.4+4212?yy=¯?á^wïû¥þÀ7çÇҒ¬À:6ÃákÀ@–¾Xéò@9Ó{<·@?·ÿvä܎?Ø+L'Œ@ ¤zž+Ð@‰ý¡O?èJ*Æ}'s¿Þ/–Æ€'q¿èHüލi‹¿éº\‡ÀSB¿îSfQÒ[¿É½‹¦¼Â¿UNASNone3FGL J2038.4+4212?½°rŠ+Ý?Ì@šD?àæ´ã¯ ¡?Ð3æ!ê5?ÖÆy–3È?ÍeUœÒ?†Dš‹Hº?•3J)si&?å7G(Õw?Ț€í0ÝT?ÔßLÞÛúÍ?ÈjïAÚ°É?°×ùó·Ï?œ-#BÜfn?ÞöKE"(?¸LÙhº?ÜÓ¶>
‰d?·ÒÉDR"ç?S "íû}?Aë}–ìח?âx~¹š²`?³žZ¬]©?Úûaø­­C?³Êüš—¸4FGL J2040.1-3137?ësW9'ŠñÀAèAÝ!êÀ:¹Åԋ0À<<š	+!í@ÐõšKpA@š(»
,ª?Í徶3®-?Á·-[?îÄùdŒW@>½õŠ±?ïq¢"¤À¿ç]tàQ¹Ü¿æ 0÷ïF¿éÌòŒyöf¿Þ†õw/¿ïÿ°_ïÉUNASNone?ïpV©«¥¥?¯¤¹^Q?cJ )ì3f?`Ã6ôcÙ.?͊›‰ð?Ž]îîŽâ¬?0=6r?¤n}k§Ò?m®vçÿ¹o?'œŸM¬>©?¤Ûµ¬N?¡öQ™ùçÀ?í)ǛéD¹?™æhªüY?‰\j> Y?yKØh¯†?³†5Þî'?—"öù?îœúØ쿼?‹ws¯â?pprK¶Ã?bQÒÄå¡g?¤"Qbê[?ŠNe Æì4FGL J2040.4+0312?ÜlºáYÀ6jǸÕ¦À:¶Ø¦ãÀ<5Cu –
@ FKé¸k@A3æÉÎ?Õjpr[g?ÑëNB-L?þ×]I‡2@St^v­Ü?ài
à"S.?ïšÅ³Ó׃¿ãúz_l¢¿áÎjüÎX¿ïû¼~Ëâí¿ïò&ޑoUNASNone?î4N»=? éÓó¥?'Éèzÿ?³MP‹[»?£o7°?šâ¯Wu»?íK1&‡?¬Õ$™5?'ø`Ó@…?˜ßnv×?°è^û™û©?¦(Y(Á?éqïñsÉ9?§fB³U@?±j,ÉÁµ?–ÿNä™Å?Áƒ*.ËúB?¡$¯e3ÝG?耾aç~_?§0²^Y?¯Õþ=Ï`_? ÅLX8?Ɔèî.m?£MÄ«"Mj4FGL J2041.1-6138¿žÊzÖî‹ÀBJ»˜Çâ'À:²Ìœ%eÀ<žÙç@/å(
eC@_ÀY÷Ã?Âz¦r	?±¿ÃúÁ'?ñ
£ÇðÄú?÷6¡þ»Ý?ïõ®£¿ÕoX½ÜD¿ã$À™+¶¿äïþ®Ç¿æ¸ž¬þÑ,¿ÐÀ£ÿN)YUNASNone?îŸñ±¹ï?™
¥"—
?aMqŸæÑ?U&!bƒv?¤ì
ÊpÇ7?˜ÀzåōÍ?íwë{u"…?ªk•Ì[º?ƒ•¦Fyƒ?‰'$ö¢?±Íï[‡»o?§/Í© ½Ä?í'S¦¯¬?"	¦/ž­?"¾…iœÁE?sñƒtãK9?°Õ––êx?âPü$Ó?ê³æ
jj?›†ûµÙö²?¥ öéE-ó?Œ`¢z€"L?¿T:º¯?šh†¢aö4FGL J2041.1+4736¿Ò¼¬A®Z@¡QÙçgƒÀ8rZ¼8¨À;1hWØ.@˙>ªà"@ÊåN?°hÀ]ӚÇ?Ó*Y— @ /ˆTÍ·®?ûË°å"?ä¡þíÜ<¿Ñh–¾•¿á0³[â~æ¿æ*ü-¨…¿ë'€!£hпîmm¡n$KUNASNone3FGL J2041.1+4736?l÷ˆ¿"?Ä?avK?ÄÂÏ?ççß"ܼ?Árútjâ?Ï쥖î<?ÁP|H)Ü?Šw@T¦†?¢˜ÿ ?çTsKї…?ÌÖ¶ýP>†?Іe®Z+Á?Ì"&t?¼]Ô÷c?ƒî'?éOômm\ã?°©pþÁO½?Ç«>í‰?­$Œ»‰|?€ )H]?bÞ+@úa?äuœ(Í?¬†S¸0¤?×>Çʇ;~?¬‡ÍIÉN4FGL J2042.1-5320?éwm ƒœòÀBãŸÂ¨†œÀ;RÂ}¾qÀÀ<·ä¼­šØ@ 3Æ 
aƒ@T@C¼î2?Ëd¢ÁáaY?"píÓ؄¼?Êg|;ôº?ýW
Éĕ?ï[}¾Ú¿æh/ßkµÜ¿ääo ÷±Ó¿â¢)?êPÁ¿ÅÚ»!ÿ"/¿çNV"uUNASNone?ïCºn­"?ŒäJã?Nf¿x"f?CXdâæÿ‹?–•|A嬙?Œ¿íC¿?ïj.ÈH¯?še!ؙ-ë?Us*
£)?eº¹€N¡?;‡†L¸¤?™9¹ð`¯ð?íçÛñþô´?'	¼_…Mõ?qšð@pÔÈ?`–®h
Ð;?¯NâØš/?'Q†¬/î?íó•—ic?"Ô9£ÛÉ?cB®ë†?[֔§˜à?¯'…Ž€Ó?"ä""qô4FGL J2042.7+1519¿ë—Œÿ$À0F[¦ïÃrÀ:ÈLÃ'1À<a¸Š©@q®óñî@꟣žÖ?ÅÒVúb²'?±ÒH·©Ïó?î¿>¿Xp?ý%"GÍÊ¿ìà‡)T ¿Õ¼­šØ]û¿à}Tß«KÉ¿å@x`cíæ¿É߄_u±]¿é\_UÑUNASNone?íЈ9A…?ª'ڐÔæ?c¯ónrÙ?UÒWn½ÊÒ?¶Ùn>š€??ª^ˆŒ?î¹W©:Z?¥|‰tØ?d=$'D\T?sÅh<?£&³%¤?¤ùÑôë8?í8­ËéýT?—g
j	àù?Ê1=6}?quŒ³!l?´Ky	UL?•¼Ù¾	´?ë‡kêfw¨? ?ëz!O?w)1n·Ù?n4á;z?Á),Ú«Ÿ? )ºRµn4FGL J2043.3-1520?ìëð/
ÅÍÀ?sBí»ZÀ;"2.PucÀ<wìÔªà@ 2¯Øu@¼Iº^5??×£e_Ö)m?¹ÂH9€?åó s'õ?þLjKù'Ê?ïÃ[Ÿc6¿æ
d(ô¿åt%kÊSv¿Ü W xF¿èEÿ©þl¿ïþ^à`'ˆUNASNone?ïŽaMÚR'?Ç‰h-Ùz?Lj^'?Xœõ½(D?Š¡'Z?#>ò‡øX?î¿^Ý]È#? \RN²?a·K`-y2?qéJ+*:Ò?¢ît ¦9?žÆC [7‹?"q?Ëʓ[âï?{+.çÎ?m¢ç(óª?ªñù¹ý?ŒÔ7+gM'?íGµPƒ`¢?•`âe³`[?t˜|_}²?i†¬]âø?´x͵ô³?•RêRœ4FGL J2043.9+2051¿ã¤zÄIùýÀ*ŽZݜ'éÀ;;øÒåÂÀ<«qøjàI@†å'Á@%Î_ª?єDuû°?ÝÝá<ps°@
e:í;Ø?üãô0¾å¿íÜiøÂ?ïÿ¨Â+‰¿Ú¢Ô`"ë4¿é\'!֝¿ïÿ×ñÃý?ÒDàPãUNASNone?íkûí4Î??¨c"`4úb?gAîÿ®?™M}3NÌÚ?ªŒz‹»œ<?£xBæ"?è.áy"?Ő@ý?»W¼3я?¼=rï×?Á›©¦ê°ç?½µo¬Ç—¢?åÁ0Q'?°à̪é?ÃNéDhû?¥–‹6ãæt?ȎúP¼Ó?§3'a"e?äƒ̖9Í?®J#	h?ÃU	ÇÖ?¨ëUЕ´?ʞÅàö?©Uî–Õ˜4FGL J2043.9-4802?ï)Ÿw:ZUÀC$O"}ŠÀ:a'W«¸€À<Á#і`)@݀$¨€è?ûChjL¤ô?ÃOÜ÷'HB?ã"BwsÔä@ob?ùó:¥|¿ï±Óým©|?ïø®6Ý¿ÅUP~ó{¿äd­³,¿ïÿÆTǏ¿î‹EC/ÑUNASNone3FGL J2043.8-4801?Ê\ÓÖ(¼?Ç6ä F…?è»ÌE˜R?ĂM%M‰[?—£¯[¯ú?˜d>ÃOê?µ_z…>t?º´r 
Šê?êÜI»ËÍ?Ī	'8Ç?ºq£,ã-~?¶ fÒel¡?µˆãkêçÛ? ´ÚQbKÛ?éØâ˜?¨Çpe¤Ú?»¶Ã».q?že8ÐS?ÇêF—Õ?°eî°Íøi?æˆ/qoÈÑ?·U¶`W?»éøSSÉ?¥:–û
4FGL J2045.0+4202?ìÄìù½ñ"¿à£öíóŽÀ9s?VW$ªÀ:ujhS@ Þ8¯õ@ªõ&ˆ*?»ŠgbèÑ¿´y€žP¸?÷쩬6TP@ÂúÅX8?×îyZ^ñ'?Ñy þ'bÅ¿ìv_"$m¿çZ"ö¥
k¿Ø*Hiü¿Þâ^D)UNASNone?µê8ÇX¿-?±ºðQ¥_Ü?"B ä.[n?–ƒ7éä_D?쨧ßóu??´ÊJ÷¯{?É@?ƒFŒ?ÅA³R?xÙsgÔ;Ð?'Êù¶ 7?é~=8^´'?Åú"‡¸?Ó n$£ç?°†ª<B¦Ã?®6ÏÊû'?•PW}êÎ?äN[ðþT?°_ààsð?Ï
ÉÀœ#P?¶ú"%;?w~¦kŞ»?oØØ®·?èPCkî?·݀åË4FGL J2045.6+2455?ìŠg0÷³À&Sü–þµÀ:í§þàEÀ<L2Æü©3@0mUÃÖÚ@¬¤¾Éç?ƽRÜEæ"?úhDµw?ËVâðz§@¢‰,d¿êµ×ÙôÓ?ïÿH 荿臦†è½¿å"‡…¿Öû!sîf¿ïÿ⾦™\UNASNone?îŠM,%ëÁ?£Oå`xó?[qd­Dô5?YpOWtœ¢?¦¢7X?¢ÿ—Ø5­?ïìÞú?«W`Pw¥2?3Pîõ/
á?P:¦iÓãÖ?Ÿ• 'ò?«(»0¨ø?ëÿ8S5/? åÝ‹ñË?ˆq3µ?uë.ù''?½ï?óçÜ?Ÿ("E5Œ?îùå¶?B?'¢;¿üŒ?au«º"H<?UÄòžá?ž­ÍÑóÎÂ?'WõÂö4FGL J2046.1-1626?ÍE\ɍ/ÜÀ@Mz$‰LDÀ:n"B€À<~3Ѿ¤@<]ˆ¿?ÿÉ>¢Òþ?ÉÐ1[‰"?Ú`?»ËÈ@ÛÂ3×@®Â+ß?é:?A‰¿Ýc5ÄÝë¿Ó>âéĪ¿ålb©Ã]¿î65{âÏn¿ïüTyÔØ4UNASNone?ã7§
Ór??Ã*ɵ#^Å?Ä/:º¿?½¤;€òÆõ?Îò)Ì­|D?¾™ 5™N¶?ëd<é)?¶ÿ½(®ˆí?¡ôJü–L?¤À1¿ò¿?»å šl8m?±….ÏCÊ?ä#R.@(?´Æ«Ô	?ËØ@¬KD?±ã[.o6S?Úvš´á?£Ë•ýžz?êçŠxÈqD?š×ÚmðT@?¥s˜A	ϛ?‹¦]ƚ&?¾	à7Ž?•®¨X"4FGL J2046.9-5409¿Ê¹?Yå­!ÀC3֝0'À;+m,SE!À<²ãô0¾å@ ìôèâÄ?úÏ÷>^‡?Ô'Jœ±Q?ΨZè	?þvÜG©ã@~õ&`è¿ïUtÁrüw?ïώH,¿|¿ãto=¥}¿ÒæV
ΐ¿Öz±!µR¿ïB¡YºUNASNone?ïB+Âÿݐ?NyÒ7‹‹?b…ð¼??YmlÆñÙ%?•w¶ü6t?Œ¥©Ž9?ï?H^æp?™ØÀÃ÷·?U,TÕáCq?cû©#~ö?%Q¦ÅÐ?˜³?~ÎÛ?íÐæßSÜ?'ý(*:6?~˞Ä:?p.hº˜·ñ?¯0¸–é¼?'R¾òA‹?í¥ª¤°ZD?"š«õ²p?r,Þ³_²?hZw©¨0Ò?±¯ÜïG2Å?"x3j¥à4FGL J2047.5+4356¿ã9pÜX}?Ô7.À\ÑèÀ8ÿ,íiZÀ:Tù]N°@"§âÅÂ@½Þ½ç?ÓÁÚ`3F~?èæÙóü¼@þÓr&Ž@²aôçž	?î_u`Õ,î¿Ôjãêv¿íÛX¡ì¿ç"¸+U`¿ïÿõÿ 1#¿ãL?bUNASNone?´Ÿ1¿
F?³ÔŽÆJ¾?­]wìÕÇÃ?³"£bžþ(?ë–6zúÁÛ?¿½LècÄÜ?µuâõ+¤÷?»=8üh?ÍÑÉZ®jÙ?ˈ^N]
¦?åÜÑJ®ðª?Í -õÃÄ|?ÊKäî/{J?©ä*\²þ?Æ"Š)¦á
?¥'ªÁçJ?ãäd:
hê?®Ÿ­%Nœ?‰ßOÂ?w85+zp'?Ô{ájph?¿bгq>B?å\JŒ¸?¿iˆAÖ+x4FGL J2050.0+4114c?í;ÓNd^¿ûá>ß8àÀ9VN>QtgÀ:÷b§K3@ˆèœa@s¾Ãõ¶?È?m©%Ó¤?ÍHMv«X@Ǡʃ?ý+Vøà&?áó!R¶¿æK>AÚ
¿ã-ðžc,ö¿æIWÍFoP¿êUÒÀá|¿ívYùp™ÆUNASNone(?µiØÃIñ?­D࿖?¨QŒÅjeÎ?£ˆ	•#dv?ëͳxðe?²Ö®ž_/£?À¸"£(Ô?µâüAo\?¦÷aê	½}?§
'úÚ?êbd¸•_3?¸çG#ð?ÅWâ°2>?¤¡"lj?º' ñcއ?—ÜáEŒ¦£?çWÓ5Ç?§°˜Û¼­Ê?¸¾îގ3©?–vFŠâZ?¿^áµÏ±?Ÿ'¤'µ¦é?èüEítCg?£AÍ_Çås4FGL J2050.4-3015¿Ã©yÒµ3ÀBÖxl"h
À;þُRïÀ<€‰Ù25Ý@¼N¡MÃ@³˜Ôw¼?Ñ{nOê?Öbºà;>š@¤³ÃçJý?ý²þ½wÅ¿ïÒ·ÈXÉÆ?ïÿLa¢—¿à'ÆN-Š}¿éѼ ¯¸j¿ïþªà"Ô?ïõfI
5
UNASNone?îù~Þ¢?—01öúzY?t™ð2&ØF?qéÌþ"úu?›©Á÷¢{?•¢Ü•(»?ëRƒIŠÌ?º5F¬Jì¡?¡3Äðßs?¨2\4"±?¼Ò;9è?³½—¯¸?é+¥zxM[?©ÄËͅ;?²÷W*Ì_?˜
µŒ2ë?ÁÕ¾€¸šÃ?££ÙK'Œ£?é‹t¹¬0?ª¨dñ­?¤|·ØÃ'?•(&Ë<'ð?IJÿ#t?¨ lÖzµh4FGL J2052.1+5539?ç|€Î¾áÊ@móùa€À:¹‹U38<À;ô×°´h@ös%@vÅ#‹ƒ?Ðt4…Bʀ?³DS§?éŽmìl¥?ü/_"K|?ïìFD‡ïM¿â¡DˆÆ¿¿êŸç[ÄKõ¿ÔÄ5N–f¿ÞÍg'ߐõ¿íäñ@õh¢UNASNone?Öô/qÑ´Ö?ÃՊďà?tÕö'[G?m­"+I&?ä\<Yô
Ý?ÃãTh]?×O÷A׳€?Ä	'ùÖGà?—¶U¢23?—yGõ›V?ã᥅½w?ÃÖwüŸ2?äaÆ:#Õ?®«ŸÒb?œÌ¿Žt¯}?'žŽ™WÜ?Õo§'m`?­0ƒÕHO½?ä¿Ë¯".¡?®½ˆ}á?'y9î|Ñ?'"¯æÔ=?ÕhÕöjò?®q>aËÒ4FGL J2052.2+1635?ã æÀ1dô!-wÀ;
Á$"À<'=¢"@rò»ÉÅ@UÛpÔ~?ÖÊð¿\£?ïAÊsbÎ@Œ¿ôw5Â@†  ´k¿Èž&܍µ
¿å²¢\·¿áŸ¸Í;‡–¿ïÿyB=K?íöÛ>)±T¿ïþùoÃzUNASNone?ìÊ÷L·a?¹ž}%Ò
?²2VX7AÍ?´Ü¨ ±?×½6Ö;?£3¬ôs
?ëѳÙRš?Ãq^gKޘ?«˜j^ÌÐô?»¬·¤Üˆ=?³¦1éϾ?·8Ä <ò‹?â(šÏ1Ú?´pØ-ñB?Ϻ jhpH?±˜«pUê6?Ç¥q*ZÈO?§×Ð)¡÷?얰›9¾?±¥¸nvFÞ?î}DtîÓ?šSó·‹æ?·ÛÕÓ®?¯D´ïr4FGL J2052.3+4437¿ï'Ø=Ýö?¶öԈ-
¥À9̌5-À:¯
•øÛ@Ì7Ž·"@"rä#*§?ÅÃdCK"8?Ý»ÐZöƛ@µQþÐU@<""†âÞ¿×°Ôßøà¿×¿!='\¹¿ç*7Á¸F®¿íÂÝ_¿ïÿºà¼ô¿í¦.}kæƒUNASNone?µP"/;?«ªâÚÇ?Ê¡ä½Z]Å?¿ÿs"
Ê?歄¾)B¨?ÂqöÇgªØ?ŸÐ;ªë?àðïÁ]?º'ÌçâýÅ?µõÅÅRÁ?ë¯$…¬H;?¶"ÛٓoÎ?Àë[©ãµ}? ¨×•;kx?ÍúÓt.µ?«‹º]<B'?äFt8Æô?¯ÏÐञ?Œ4'Ùºòÿ?t½½.Ëþ?É5‹´°ö?¬€§NÕö?éA앫çö?­ÓÜâB•4FGL J2052.8+5739?ä~¤Põˆ@  ¦°)(À:ÉÈ5ŽWÀ;Á¡ùºk¡@	ý½/ ×@-°ê7?Ä驼ÒXÓ?½½Šåv¼Ë?úB¾ÁqNø@V¦í•?èç$œ—zÛ¿ã¥jÞR¿é·à†=¿Üœ›PÓØ¿ëùoÃzn¿ïÿÚ €UNASNone?á¥EŽëq?Á†#y?«¼–_‹ä?¤m½T¨?Ù=â,b?Á4þD£ö?Ûo]¢@k?ÇX"úž`?¦àgªqT?¨®Õþo{?àÚJ´8µ4?ÆÐZ³žbš?ãF¯ŠÏ?¯jÿk•?³!u¦žxû?™Øס¼>_?ÔªDiD:$?­H‡ý–ÿ?䳉PÎN?§²oÁ_Ç?·#£ÙI÷b?™iÐq·"?ÐÐí÷åŒ?¥Éó™œÁv4FGL J2054.1-4054?äJ_!x ¦ÀCö FÇd®À:A…ô¡'À<_Öq'<Ô@´6"¦É@"*ú?¾!-¢$­‰?©s€Û¡k?낎»F"@n_.8Í?ïW¡!MW¢¿å'"¢‰­=¿çÞDÄU/¿áwáî-¿ïær$àŠ¿ïÚ8?ânUNASNone3FGL J2053.4-4052?î‡7¬Sl‡?·î+`µ{	?†Éz'í'?­¦¿Ç&?¡Ú&±<5?±Pªîyd?îmv¤Û–Ã?¥ÿÍÜÈD?uî¾!	Ö?ˆˆäHK:(?¦j½î%Y%?¡NjÝEó?í=W¬Ëøî?™,Èéãá?"]:+¢nM?†¡^'À•n?±=ô·?"ŸÙuN;?íӎÖ_Þ?êÀ£Ù´Ä?›£^€Û}Â?†°¾Š£9U?¤õo",C9?…NKœ/4FGL J2054.2+6904¿è}æW.Ý[@.'ÄupÅÀ:Lµ›Wß»À<Eþ7¨ã¹@&˜®²@ç~äâmH?ÂF­¹a5$?Øó;Ì@ O‹XŽ?þo'€EŠ¤?è(wŽ'ÿ¿Ä®QM¥¿Ý·A 3fµ¿é'Û¿®×¿é"'?h¿ïÿƒ9UNASNone3FGL J2054.3+6907?ÁZ¯¾Ó£Ó?²ñѼº$Ì?ܛ+뜕?ÈDˆ°°Y&?Ú·|4ù™?Çd›¼qS?Ñ…]D'?ÆDèåJ?ߕ~"Ch½?Ì	¦Üz
L?ÎÏøn¥€?Ãö×¢©Œ?Ñ[aŠHù¶?±]±¶[šœ?߂&ºhtÇ?¶—TÀÆ@¾?ÎDïv#?«À$gVí¢?Ò[»€hU?¥muñHî?×?ªâ‰Æ?±0ßý[*r?Öd™_ѐ?ª?™Iäš4FGL J2055.0-5218?í/MܒúÀCèA¢a¿8À;>$'ýuÀ<‹î:ތ@¸ðá©þ—@ø&"»?Õވ¡y·Ò?Ñwûd9æ?ú«~3Æ@؋`pÙ¿é'Æýó¿½8¹›¿åãEf­¿âÚ
ݹ.4¿ïþÚ0bž[?ÏJùãÜ2ñUNASNone?ïšXgxøC?ˆ­^)û?Nûd¹ï§?R".Eç?‡‰ÆkvP|?‡`h"T‹'?ïc4€ªD?'òB¶ã?Jྶ™ç?_òû²»÷&?'ÂoÜÁÉs?ÐYÞ@`?î÷Æ©F3?'›E–T'V?ŒØ6‰Ô?Ә¶ÄÐ ?§šƒ˺W?`¯Ò¾h?ï•8ӏ–7?qýmB&N¬?Cã#Ä©pˆ?9É£ú»Áô?‰s˜ßÏÛ<?q‹JIF4FGL J2056.4+3142?ï«'!=M¥À!£;u!MÀ9<›õšKÀ;»¹&&Û6@웺Iì@]!ê5"?µðR

ú?ÚÊd<Àz¯@ ì'éSQ@gŸÜ~ƅ¿Ô>$ކ³Ž?…¤éó'ù¿ä-–¦ Z¿è±càO5¿ïþ®û*®¿×']<9UNASNone?ž"Ü(•Ñ?™Ct{eˆ:?êû /'(?¸|]Xg"?À>ýrL×?µ‹üxѼ?—=ƒ±|fc?¢µîÆÆ%¯?écoÚ}¯ç?Ãå¨ÐÏá?NJÙ³—?µ°k¾?³
gÇN÷D?žÂÉȌa?è¶#dÈX?ªHzì"òÉ?ྌEc?¢ûÿ‡r†?¡³‡¼š—?…v/
5?èúÄb"?©ÙÓÚ
š?ÇўÞÿO?§¨%DL{4FGL J2056.4-5922¿æBi÷ë_ÀCp¾´ .À:]¹À€Ž0À<yµIc @˜üsÙk—@Ý_á'?Å6ò…n"?ÉOJUŽ§Î@¢¢&0@u@ãJÇ?ïòÏàþ]¿äøŽ¼ÆÅL¿ã"xKtÈ¿áÄ x°ëÆ¿ïÿíöé	¿ælQaòc_UNASNone3FGL J2056.3-5925?î#`|%ËÑ?¢os+'Ä7?Œ0t"ää˜?ŒMŒÌy)Š?¦½Û4ê	Ó?ž`µN1(ò?ììñé|D?±ÿaü ·?ŒS#TM°0?"á.úVãÃ?µI"%~?®æÎnÿµÿ?ìAeÔaË?Ÿ=œ—"\†?›ôÉФ}G?‹Ÿ:nüÐ?´˜Â]3ÒX?—×GÀÂCÎ?ìßÜ-Uc¾?'çm÷Ñ?œóŸ‹ê×?ƒ}/s±…‡?±Ä6²g\?Ï­éˆ²Þ4FGL J2058.0+3338¿ÒaÖÙ.ô¤ÀU´$_ZÙÀ;-¶Œ§—À<¥"²È@ƒŠ'3õ@-@«?ÏíŒàΌk?یÒÁƒmˆ@	.<b'?ÿüW¯>q€¿ïÿà iA?ï¡ 8Bg?îN™á=@¿âåÃ=×Ñä¿ê³"¢Ú¿ïæ^£úE¬UNASNone?àó2$A¨?Ä'n—
2è?¸™—± ?±ÞR(^™a?×ó5Ë·ØÇ?íš^f>?Û=üÏL?ÍsŽ¥?¥bByr'?°×/ú–Å?á{tOc7?ÌìºLyiæ?ä®;1u?¬±7¨öùê?¾–£\¶¯ß?¢@'6fx?ͬ/˜·â:?¥'žÿY#.?æSçé$C³?¹vê*ê¼?¿€¨j¢?¹ÅS$‰TË?ÃðàJƆ"?­mµµÕ€@4FGL J2058.5-1833¿èRT—ö›ÀB¨ÁTɆÀ;÷sI£¸À<Ý1=­ˆ@%% _Š?ôÝWšÉ?ÑÇ"¾Æϳ?°U2a|Ú?ÑwÂd$ö@j&Õ+ëì¿ïÿõMõVY?ïÿ2æY¶¿ïþÛ½«q³?ï÷݇/3Ê¿Ýí¤2϶?¥'mœÕRUNASNone?ï–xÕ=fj?"#N^`Q?/C:M®K$?4xª¨ªÚO?‰ä½Ço¬/?'÷µò_Ž?ïN»i¸N?¬ÔmQ	‡0?EšqÍ¥ðã?j·¤	 Ò?•{¿:&²?¬q­k _?ì‹_8˧T?¤3¡å	ZÖ?iåUGà(Þ?`'Ó"n"5?ºÕۏcÄ?¤)qÊ?íFBꂖ?¬«âq'?hÀÀ¦í\?ra¡=ÿô°?µ	Ղ¦³ð?¬ˆ…ù4FGL J2100.0+1445?ì=-;¼2À3üæâ!ȨÀ:ŒÙ™cé´À<@HÊt,ù@ç®Tçî@…¢Ëqƒ?҄‡ƒí_ê?ß5ÿ–Mµ@È§¤X?÷̧¨.]¿ ÊŠÛÄ?¿àåê«%)¿æ÷çÝõ>0¿í'E.Þ:¿àèú}	@?Ì$ZR[ígUNASNone?êý(m?½	''7ä?¡~»ã"+­? È–Hsk?¿WaÒͱ;?ºÝ6ºn?ç®ìjp»·?ÈÃ
p0¥/?Á5¡ñ—dÓ?ǎN´åÙ?À¬d¥¬S?¶õi-ƶ?çK`¬Å¬Ý?«Èè¤Db?µL-ر-?›¢j!k[v?È,f`Úsó?¦núÇ1Q?àttn/Ó¼?µQ¬Ý
ó?ÈÓ[Ô?µéGÊ>?Ò­ußn~?µö–¬4FGL J2100.0-4356?֗­˜v{TÀDŽDR?gõÀ:{®•ª ÐÀ<s"vD)û@¢©"P¯@Ì"û­Šè?Âă½B(?±äÖ?íÛ{@¾>?öÈ¡›@
¿å²À?à¿åN.â´G¿åCì>Bu¿â.'Z·Ü{¿ëŽ'Èê¿ý¿ïÿV"tnUNASNone?í@»/§š5?­5i‡{¿?rÁbaî?h¢@Ó§Ã?´Î\ª<?¬þa"ª©1?íÉ©žNã?«_ˆ"G?}íXÇt
	?†ŸžyŸ?¯§»Œ.?¨¾aoÎ?í°îþ
?"J²;l¾>?Š¨ðT°1?~¥©‡»­3?®oeÛÚÓ#?õ‡ÙAj¸?ìšÿxGo?œý*ôøJ?›yt¡ì?‡·áW€?´I§
D?—OkÙsr±4FGL J2101.8+5044c¿í–îïaw@½šzj)jÀ9ˆÁe}'À:Ø´«m×t@˜^IŒ¦@"¼¡Ÿ?Ñjþ;.Õ+?ҁõuü@5" ¼8@€ˆ'tð?ï¿ø="ßE¿ÕÔ~œéf¿ç|΀2À¿ë8–IƒÑ¿ïúmN·óø¿î2í"ñÚUNASNone(?݈WbӐÃ?Ä2›:e
ï?¤äQ#žŠA? ½j"y7?ßÛx¸ö?Ą_^ìq?É=pC
&Ù?Á¬¯dOÀ?ÂvïW0¢?Á/Áܛ—i?å³fê!?Æ?6öÑç¤?Êúé™æ7Z?¤(Imó
¶?ÅÖc­œt?¨d^Óó½…?ãˬ®U%?®Ê8ô¡©3?±h™‹ÝV¢?".¦×=*?´ւ—…¬?›?»R¯47?ëPþ1dw? t¥Ò5÷}4FGL J2104.0+4623?îpžÑ;òJ¿Ôj"m¸j?À:<»+º˜îÀ;¸–ªÑÐB@Îäõãq@:µå)»?ÏUöV³ëÕ?âVr¬MÑ@ó-¤}ù*?ûrA>¿åÜÁ6–•¿âiOBÇ%¿ÞKZÓ¿ènq'yAŠ¿ïÿÿ" 5•?ïðÔ^;Ÿ"UNASNone?Ë䅈=by?ÁV¼…—4å?¶ûbÝü?µ¹"oÍÌ?æC<~"K£?Ð/ó=šÛ?Å6J8‰ ?Ä}ú4pç:?«Ÿ¢?³
/ûAê?èøˆK—¼÷?ŽŒYб©?ÐÛ¼n³?¨Øy>0¿q?ËϐjÞçÛ?©eºêÿŒ<?àž=­îÂ	?¯ðÚ@'~ž?ÑÀ×¼°?³bý"òŸ?¿`©"¡¤?©-"Ö¸é?ã'ãoÍs?¶±*+/ÕU4FGL J2104.4+2116?é%íÙüyýÀ0ъeI/õÀ:cÖ1riÀ<3­¬v0@ &J4'æ@çÝÿú÷ƒ?¹¸‡E"©¿ Ëq>AëC?èÑÌ`–BÍ?û‡«¸°¿ïç:ÁòÔ?ïþ|ý׆º¿èktøÐ`Ö¿Þ±ù⯍!¿ß­j0öB¿Ø0~ã"õUNASNone3FGL J2104.7+2113?ïvd<.Ù?Š]ÀbJü›?\Õ]«ãg3?UµT@©
?ŽÌE>Ò¬ú?ˆ¸ýû''?ïD~Pÿ ?—,D`S?Zõ0»`?pKüR¿jÉ?•ÀÜ,TZ§?•Uú]‹?íF:ühœ?—Åð]êñ"?í«ŸÞµÎ?q7?Ù»W¼?³r«Ðäf?•áǍøT?ì_šŒ0¾?™3õ»T
?•wàü'?6?""áBá2?·¥3_u'=?—G¿zB­†4FGL J2105.9+7508¿ïþ>i'™@2S^"ñÀ:+Õ£5#ÎÀ<8(¾e*ý@5¥›ÛhF@"}ÔA5?½#qõáõ?¨_¹<æÔû?î˜p9Mÿg@y®$û¿âßßÏp¿Þ)«|ñ¿æ~"4­†¶¿ÞàÙ>Ú[¿áíks¡R¿ëZsž³3ôUNASNone?íãðóÝ??§ÈT›¦!?{ˆÞc_oÐ?n,ÊÊQÍ?®OÔõÀ x?¦5yêo?î]F;äùÛ?£®N\äH?zR·«P0¼?…¸ps½m×?¦áELF\5?¡–Íú
p.?ìÎ6øw.?™W'j«?‹‰UkND?xÆh—y3Ö?¶''Ë?–š—·_?ê>.ãðŸo?¡5qcŠ?œa4,B"?"¡öÂf´‰?Ã{"é·ùþ? É2ëø4FGL J2107.5-1507¿ê'#Ë®ŒÀBn;ÑgfÀ:ø0ÁhëÀ<2¨J6"÷@ ø(›)½@՘ZÕ8¬?ÂaÓY®Çÿ¿»¹f®_Ï?ýî}÷|¤?û}/և`²?Ò¬æ}wúã¿ë¡É¿îZU¶ë¹ø?ÛlKU‡¿æOËàÏ»¿ÃàS<h5UNASNone?ì0'ý<Ôß?º:rʐpˆ?…¾Óþߪ?•ò·/tË?»Æý;™}?¹;#–,ÍR?îDz'Þ'?²:øf¸Ô‡?~Ý lfÿ&? åV.Ò©è?§Ü¢Ô‰ÿ?«;÷Çp·?ìXx8Ã?¡SÓu…nW?‡Oý3/j=?yÛ£g'	á?½U•ØLš? gÔäêÅ?íq0 7i?«¢ì"Év?ˆaí/H?‡•¶+ÜS?µ;jZ€žË?ª™ ÐøC4FGL J2107.7+3529¿½Ø£ðŠ—À A_ˆü"dÀ:~¶H&	À<
ÿÖ"î@P@".þñ@È"ä0–¡?ÈzyBáüà?¶ÖÖ»ãñ?ó"Gö8Öá@  BU:?êDã߸⵿ٍDv§|¿çM}ŒGÌ¿ì	áàÛ!¤¿âƒŽ_©³Ã¿ï«a]*UNASNone3FGL J2110.3+3540?ëó:Oã?±žà†û¨!?gÖS'|sü?`´»'?'?¿§zçsÝC?±pÔñÄ4Ý?éýŠIŒ™È?ÄLcMÚXD?V":K¬j?pŒåäu:F?ÇÜ®dψ?Ä%"8ñx?ëÌáÀÿ‰ö?¡=•Ú
Ž®?‰Æ¨'8ˆ?wpS%Ò¼?¾`ç¼ f?Ÿã·*ìÎ?îþ˜3(@²?øK'/?X†2£'‡ç?GÑp!:?ž¤–p¾Ñ?C¬vQD4FGL J2108.0+5155¿Ýúø!h@N>ò"{À8í̙¡&VÀ:vF›ÅÃÄ@©PÑ~¸B@:ÙºñØö?À\‡ÀSAÆ?ÐßüÉï£@NÅ£ßâ@
¢›Jõ¿ïⶮ}Vm?t¼j¿âþÚÁW"Ò¿ècê?ú@ù¿ëòpK™¿ïõA?æIöUNASNone3FGL J2108.1+5202?°½úYßÜ2?¦dÎQ_o&?ÔDCP'þ?ƺô$¶?ãÆ8"ð{?ÈCÝk''l?´ ÏÛT?±ýΌ¨H]?ՕØøòò‡?Êm½!Ëž?â¡ ,‹R?Éã¤â<?¼áŽZëù?ŸŠ›ð2?иï.ºÅ`?¬¢/‰ðLÑ?äV¦—?Ñ?®_"j"2?¤®¡Çöu#?Žþí*?ÀL6'?¨Eîä‹6?ê®z‹$?«1¹«7;4FGL J2109.5+5238c?ÉæÁÚDHs@	ݜþ¨çëÀ9W"¥>ŠÀ:ÄXÉűP@]±°ç"ø@Ò¹ƒCì¿?ÆCß=g¿'?µžÃúì?ñݸ'#Zx@DgE‹%?îè¹AՍf¿å%nN'4¿å÷ìÀÞ(¿ç¸Û^
!l¿ìӄABÀo¿Ýޘ|84ÐUNASNone8?ºµµÈ¨»ß?µÎî\=z?œaßW`?œV•*É?ëÉ7ð-?ºÅÎ!u ?Ó5~ªQz?Âí	~dàä?¦œCuúô?¨÷ÝA¬ ?äû|Êów"?Âúøú|³'?Ð3kæM=?­H¦(8Z?µgËVX?—`…88ƒÔ?å9P«Ö¶±?­í!ŸƒY?ÅI¡xšœ?£Iµ™4¸?¢Ž¿\"u?Šor´Y?鄫¢ß²?£ð£éa¢å4FGL J2109.6+3954¿ÒYÀgÛþ»À¹_í¦a(À:lf»ö»´À<PÍwí@"`´á¼©?ö)`F'µ?ț	›µ'À?ÔÜo×ÿ0@f}þ2 f@hH0p`:¿ïÿ&DÉ^?ï÷
ø{§¿îÃ`!¨Ç4?éìu:'Ä¿×C­¿@r6¿ÛªŒ[¨¾UNASNone?ÙÈY@¯‡Ë?É'´Z°<Ê?"fBQ{8?¥€<G3¶`?âx¡M`?ÉC@{ub?äÂÖ*¯Ø??΢|¹¥ûª?q€b×ÛlÑ?ŽËm¦¢Ê,?Ö4R@áÌ?ÎGm¾á?ãÌ£ÞÒâç?°ŠÒg³~¼?².RÂ=â+?™h.©;
¥?ÓÛ#'ÊÁ¨?¬b°Hô'?éÚ§¡<áf?µînM¯s†?"¨Ðöœ?œå¿IF'?ÆG\8÷ä?µ3iÿ¿€4FGL J2110.7+5129¿ß+,Ñ;¾¿@ƒڐڮÀ98CEÏíéÀ:aÉí{ì@À•ý­ÀB@¬ dŽõÒ?ÐÏòñúƒ¿?ÚiÐ1Ü@
ïB-¡ú?ÿdÃo?ïÔ.öw¿à†h>ح׿èö=áâß¿í֎ín-¿ï÷/væk?ï²Û‰þñãUNASNone?É·g1)Í?Å.Ïûý®Å? tzG?£ýPmëb?萮óÑ?ÇlzÛ&?Ån3À€?Å|ºï…½?ÈXnH?ȑFҐ&?ä¦5×}Ù?ËìS*YÅÈ?Ç£1©°?§ÛdûÛGÖ?ÅÿO;/8V?©Ð>3,±?ä—_ÑIÅå?°Cš®0â?‰âÙÚH'í?x9ðð[¯?¶¨'HìÛÃ?¢õÓ{¥?ìÃdOyCè?¢ÖcržÈ4FGL J2112.5-3043¿æ3U}"‡9ÀE8Ɔ"ÄÀ8¹}'âïÀ;ûK¯Ri@æDÖ ³?ù?<;±'?«é³@pž?݁b ß9@1== ò¾Ï@'wVM¿|¿Ý¸çì
?¿ç¨eÜÔ¿ÄTÌ '¿àã|aO{=¿í/à˜[¬¿ïÿý±q&´UNASNone3FGL J2112.5-3044?‡»k]6¯/?'¤iô*#Õ?ï$!"À ?¤$ô}(?</rÅ	?˜±å¸Âö?–³ÛF>¬ü?˜âDë²"?ìù欘E?º5¤–Ø
?²Šùù' ?¸i™—uo?›BM\$j?í¦¡-±Ì?ìcl?û¢—?¡ù'q)Ô?¶
©"3? Yf3ü›?]7õè7ö?VìoèAË?ëÍ:f¡É?®é¾ágWµ?À©¼y¨m?®¨âãj8õ4FGL J2114.3+5023¿éUÊ5ۍ?òaKßÒcÀ9n‡–aÖµÀ:é×5Ü@£Dîq6@±3™Š€!?ÆÖáM¸E?ЫÈÛ¦"d@×"ƒ¸†Å@¥¤ªCàÕ?ïvŸ~µè…¿Ý[òú³åË¿Þˏ(ýO¿ãÏ¿®2¿í¾‹Ái¿ïÿ ß‰
UNASNone?›œ¸•o?vžikç?§Þ¹-¯N?¦ñ[sZkÝ?í¥.¨|£¯?©Dؘè¾ò?½§d{ÁKD?½ñ³~¨Š?¢yëÝ' ?¥þäãÅá\?ë#t²µ\˜?¿Y,6#?ɄïVal'?ªN[Jº¸?Ã÷E
ïö5?¢Y[؂?ä ò竧N?¬Mis%,Ç?·¥p•;k?¢vX?§V"HDÞ?"h
!ƒ•?ë•è¸ÔD¾?¨ªûÅâË4FGL J2114.9-3326?֖oP£d&ÀE¬§?tŠÀ:Xš`hödÀ<QuÍâv'@¶²}k:·@¦¦Bˆ?½~ßrۄ¿â±†J‡?ÆÜô7Iî6@»Ÿ/Z·?êJ7&úƿ֔øà|-¿æZ*M±c»¿Í"‰ê}7¿åà• ãû=¿áÆëvÛÿpUNASNone?ï…6ã??W¶·e?a3N %{?T f&Ÿ¡Y?›û¯_"?IûNÐGƒ?ï‡|.dPò?Šõ—¡jº?<ï"åç?M­ë.ƒU®?@Têě)?Š$!Gðs?í«Fß½|ª?"ƒÈV'&?|zXgü&ã?gÁòŠì3?°Þ#{"X9?'øƼéÛ?î‰æoèÉ?"€a"Ma?vÎTœ÷?aÞIä*N–?¤‡ÕY1Ԏ?ƒ†°ÞÒv4FGL J2116.2+3701?éüŒ<'½MÀ ®˜ÜÛ7ÊÀ:"܅§tNÀ<=èõ!­@&*yPMö@ê#×u?ÅÒîNý"?ìZ0Fï©@"­`ûH?ùk5X'¿áF´"×j¶¿Òr‡[ÿZ>¿â7WOr.¿ì73"l;'¿ïígwžZ¿ïÿïXzUNASNone?'v¶R(>¢?£tI>«>Ë?çLRJý?Ƥä$¦µË?Ð?ð»'
?ÅÞ]˜n÷î?'4Ì;•|? Ã½ã>?è¡K†óRJ?Çe9JÈ?Ë48\ÀV?Æv¹£3h?¶þIGØÕX?›	2:Á•Ø?æ~'ιY}?®$Q	óó?ʆ!./]?§½ûØs8I?u*Ñ9Üڀ?cËõk;?íòs²3®'?Ÿ¦iW³*e?®3jµ‰'7?žu—ò‰ùÉ4FGL J2117.0+1344?Í€±|uƒÀ7Þs×ÛõÀ:{Ì'‹_DÀ<Dô·ÍaG@²‹'Ä
6@=¢ø½ì_?Æ´©Ýßo?ÖÙ`®ìg@ìJ[mäà@ÃHïÝóç?íœK9¿áx¾'²!¿â<۝Ëœ¿ã¢–b­tB¿ì±–`)5ƒ¿ïÿÿ«FjUNASNone3FGL J2116.9+1343?ßƲ쬖?Â	RAiõ?Â}LÕMm?±â]–?ú5?×8½¦¨¬´?ÁPï¤b¼!?ì‹o's¢J?²î¦ŠlÊO?šF2ðM"J?¢)ŒþZ?µ÷0OˆÙ?¬£åW^"Y?䊖`@x?²šžt(û?źþn©¸z?©Ï-Îú†T?Éî×7ÕE¦?§7GæVóW?éQ­ã¨?¡)ºþ¢J?¥±rÃr+?ˆsÕKMW?Ƃ^ìkæš? 3ÙGÕ ö4FGL J2117.1-5307?ͺфŽçÜÀE~\|ؙÀ:ˆL€À<'|»@ð–ºìû@	­þ«l*?Á¡ËiM÷?´®!7?õ­·þßn@o¥'(^?߬:›‡Z}¿Ñ¢[Õ¾¹¿æSþÕÞn¿ÑÆU#óпä¢n>÷âz¿ïÿ²gƸ·UNASNone?ïÞ¥-Á?e²äÔÁ«?@­j'{?3T^
×:?mÉ7¾M–?dí+F±ž?ï£Ô¾ £N?…ùHÀåÎó?30Dæف?FëM¤µ è?†qN0 c÷?…N?£sH?ï#A$Xaé?GÛkèWÁ?f?˜á-_?Y›†ˆ¥ä?˜Ïùם
?|ÒlØZ×ê?ïRN<üï"?t¢Õ•¾§?g»L¬@Š?RC°vøÕÌ?'Õ ö̅\?s•\/¸*î4FGL J2117.9+3729?×DÚwQ½"À ŒFŸ¸À9žY …F%À;Ù ™hr@}xåÄëW@8J"xÈi?±«HÓ=?¿Téf`‡)?ûMÄ(¹\®?ñî¹Ç—¹?ßèGœÌ©ç¿áJ™¶õÊó¿àÙ๨¿åÉ£ý˝M¿íǍþZäR¿Ã·¹Õ¤6×UNASNone3FGL J2117.6+3725?Ç>›âói²?¸¢ÈÂëq?¦–IÚ^ñ¦?¡l°ÏP±?èÆôi6y?»>cf[µÈ?ÑH÷ù¢Ë?ÉLÌĪР?¿wDvƒ¦?ÁVŀ-D?ãl›t³~&?ËۉÑQ{?ãSÀU'bU?­›lï2?¶šïÅ×·?›ÙzžÅ½Ý?ÓÑؘëÅh?ª3k'í4?Ûß]Çö®î?®üçÿSãS?Ê	#¯
ã²?¬måA?×`ƒß8?«ºß‹ªÇ4FGL J2118.3+4055¿ê\	'âÀÁ)/»¯À;-î@ºÛ3À<j¦'F•ç@"OÄÄÂZ?÷eâ}8:?Ӟ)`ÌsŒ?Ó|]ž–¯?þm‹ÕÓÝ@úÐ<BüT¿î‰
€6œ¿ïÿý¡UûŠ?ïÅ!ò6?ïÿ"ÕåzC¿Ú×ÄØ6¸¿å[ח+*PUNASNone?çÑKã?Âæ˘ƒC?h¥†¡mñ?bHô" V?Ð,ð (?ÂÖÒíWµA?彟Ýû)d?Ìl;HÖ?]U»"ÙÔv?‡¡Ñ« #?ÔgjˆæÓc?ÌC{X	?çŽ×ª*¶?¯–y¥ ¨?•â¯Ÿ(s?yÞù>º?ÏaAc´?­ÒMpæ*?ía±Êóª?¬ãèÈ>ây?XÓ¼óÁø?cÎéë?´"+}Ù^_?¬á
ùŒ4FGL J2120.0+5257?ïùÒg҈_@[©ßaúÇÀ9?踻ÐÀ:àF3À÷¬@SN×(›U@äõ$ÚªÜ?ÆF—i¾?艀qÕZ@"·þ®û?ö?ÊÎDò?ï}{áwÔ£¿×ïÈdÞ&¿áÅòÞ.t¿êûÒï)¿æÄþ;â¿ïÿùµc#¼UNASNone?ړ»È wú?Ãi|ÇO™R?'0ž»
1a?ƒù˜Ì©?â$&Zy?Öö£´?ÇÿÞç¬Ò?ÄFá"?¼Ÿ›_úÿ?¹û4d ê\?ælÚ:'ì?Ǚ5MÄKX?Ñ?B'cä?«Z_Š["?¹`‹ïÇ9ö?šØбÝ1?ä4M{ófÏ?¬;³ñ­?¸U–cë`?œv͏7ç·?À"ÒM?¥‡=#;?èôÓ-oŽ?¬´ÔÂÌ_4FGL J2120.5-0138?ïà"JäÀ@¾&ÉÀ;9'ôcê‹À<ž3>íÂ@!ÞdNß?þh7‹‡ˆ?Çh1ôo¿‰Û—.ʹ?ÃfýNÉ@$`Ρä¿îâÅÝo\Y?îY¨¿ãVöâv¿ÞVé†@÷A¿ÓÜ:¾l⬿ÌQü)ÝUNASNone?ïÞÛÜ®x?n<¤k1"?4*óµ6/?b'Á<]?nžáER?g™´	ù´?{@ã?‰ãä]ä$ÿ?3vm*­\ì?Fle(ߑ?Šv­¶Ú\=?‰GzH2y?îPvqùD·?Œa7o´?j«ˆ7WŒò?Wyý°'b?©Mà\ö;È?‹—ï¿ô-??ïC=säÃ?"èöãÞ_?X·A—Iç ?P_èÑÕ¾?ž,$8ÉG?"s_x,C4FGL J2121.8-3412¿Ýg–ÀFp(€QÉ÷À;É%,à2ÛÀ=*"¬ÊÎÆ@ £~‰x?ü—£U>S?Ú¥‹-lË?ïþáQ¿u@#È\$Ä?ý=ÓLKˆ?ï=è΋î¿ïÿõƒ¥;Ž?ïþìɹ¿Ãbý±@¿é3çcQ¿ïî´³ÑSDUNASNone?éÝzCÆ;œ?Äééëßã¥?§˜"†}n?©~p´ó<ß?¤OF²7?Âÿàéd?ã×A{óZæ?ÑaÖ/3¯U?Ê2í¢j?ÎcñÛ&^K?Æ Ç#ñû?Á5¥"¶Ž‡?ç®~šÌƒ×?®n¤Y¸A?ºaE¼îf?¥¯:¶fT?Äcoyr?¦_lB²½T?ÚVyŽ'ŽJ?¿Ša‹¤©d?ÒÄæ~_ö?ÃH®³
Ø?Òån‹ZÁ?½êÒÔ«'4FGL J2122.3+7653?Ýöb-­Éc@2²IÂÁ±À:ù» Tž¾À<{:r•@0Fþl,#@£a~ ?Ëüð@šNö?Æô·7_?úk©f–7@ôÿý²¿ïÊ,¿%Å7?ïü% "Ÿ½¿ã[Š4¡È<¿ä®‹™%Ö¿ãÁöD•[F¿å™Ž´/óUNASNone?î Ó¹ïo?¡iމ&tª?ý"'9>?€ÐŽ}m+C?©s|ü#ºË? P¥€íäŒ?ï:c(xŠ¹?''CGn+?c"nyq?px¯
z‹?–?êp€Ù¾?ÃÓ?íj?‹"mH?—Q§Ït½?Š-k)a?|­.˜…ì?±hV>°t¼?"$+_N£+?íЗÙuŸË?"}kÓw?Žd~*Œ_Ã?yÌ'gô­[?«]bÞëV?9)^Û9Ò4FGL J2123.5-8315?Óñ¸™äîÀ?$-òˆHÀ:ÍF«µûÐÀ<7™èsò@@ûEاK‰@¼Þ…[ôó?¬DµÝr¿£îî¾AÍ3?á3W{V@¾'$Ý¿ïýýÇ@›Ò?ïºa¤µ¬¿çÅä Óõ‹¿ãÝ}‰˜š–¿àì1¡¸¡ó¿à·Ð]óÑUNASNone?ïvSõ@ر?‹7~ŽCÈ?c[‡O—ÖO?a+FAê	T?" ÛãÞ(?ˆì;à1?ï"m2¾Š%?'˜;^¬iŸ?6´¨¤©Ù²?Hû$q?Ž/8('?'_—ñj×?íA{™Í?šª"-…Ô{?ƒ]§,?ts÷uLÉ?³'[~RÖ?˜E°ëµ£?î¤cVó!ù?†Y Ù§m2?j!NØzh%?^=A®ôöÆ?¤µ£F9ö?†µ¸ì¤4FGL J2124.9-2433?ÙÚÿ1›OõÀEå.rÚ0À;sjZç­À<‰M DC&@‹/ûh@Eˆãhð"?ÒÞbKy¦?ž‡ô¼¼²?Å8L7;*£?ûB"°Ìf ?Ë<*'ÆÃs¿êÍø{§@K¿×úÉ?#¬X¿æYlÀd¿ïýñg¶È¿ïæÿ8mUNASNone?ïùO^˜?š¸Ýõ¬?R`50øn?KZÓM-Kð?›¾
ÒÁ}?š}3ׄ5¿?îÝ5"ÛZD?™÷-tþ¯…?`‰Øb‡«?l¡`rŠ'?¡"ÎÄ3J?˜‰–7qÈ?í'`Ù
Ïý?•.Á$Ã_Ñ?'
°V?…F&'ªÜ?®Ñkìúù?cÞìÅ/(?í÷šyÞ§ø?'žEW,?{mÀËl?pê
s1§=?­$J¯ýg?¿<"Á3Ü4FGL J2125.6+0458?×kò¬À>Ü@¿ã°>À;Në¯æâùÀ<˜%·I­É@ ü´fú`?ü‹Ë*5]°?Ñý6aé?½¬ ›$´?îƒÝo²@?þH%Ûܵ"¿ïÿúVrÓ\?ïþ½_ÇeÛ¿Ïe
gs¿Â%›¨±:¿ã3ÁˆK¿ÙZã¦XUNASNone?ïÌô" <Ó?pۀŽb¬?*lâT˜!w?!)\Žs!?x²‡Ý<Õ0?pª™_H·?ïZL—æ£?'3NÀá£?Eéº²à˜‹?Váâ֍c[?"-¨æÙ?­¾µ…š?îPôZv ©?‹'¿Û?pfÅáœ5?dÅ?îø¤?¨ãáœjs)?‰³á̖?îðŒ(Ó0?ŽÇ&
ƒÃ?lzqX"?]Í÷0Ñu±?¬YU–a‡{?Ž	f
¹¹4FGL J2129.1-0240?ì™o{VÀAðuöý!ÿÀ:«åüjIÀ<=²¢i@ƒÉeeà@ÝäÅ©?ÈTí˜oW?´˜|c'í…?æÞ|Ý¡0g@	j
fEj?ï°~¿å±ú´f¤¿èf££׿ïÿ¬óéqH?ïût_ÎFÊ¿ðUNASNone?ïû9Í6zJ?AñºQ›,À?áS<7`?• '‰å
?@|¨{¯QB?@£Ô·Óä?ïM"gbT?¢À[te™?\)P?~.MFö?"PŒ±Ðs? )DLÂN?íÝð›Och?›ˆiV´?r蔷óÀ¥?sA•sÄ?¯Ãã´Q`?šÂç¦ÕAf?ïÓ ¾}¦T?qZJ8€ ?wB…ÀK?Êm—õú?uø²<!U½?q@öÒ	4FGL J2129.9+5833e?ÅûäIb–ð@U›¡±–À8¯Û$~eÀ:Òe횢®@ÒqdFPœ@)Ưc/?³Hª~CQä?·˜¤Òód@ÏPB7²õ?þk‰0?ãÆ¿"9C…³*¿ÝÐ&^
§]¿æµV¬µ¿æéìb"IÏ¿äÒìnºÉ?³õR'AUNASNone3FGL J2125.8+5832?¤hó68e;?˜RÓ'H4d?†X®õ4'?ƒ û\+'?îa7ià¤Û?ž©µw9?ÔT¢²>?Í¿Ñðùo'?È刑1ðB?É1)"Õíƒ?ß97SU¢?Ì©©P&V?Ñ÷7jv?®Lâ˜)?´Ö4Ñt*–?—¸PÅÁ?äi¸J? ?®œ›ÂÝ:š?Øf›×0P?¹ôq?æi5?´>¥— Fr?Ÿ²Tã?áDÝaß	?½#`kæ±ø4FGL J2130.8+2649¿v±W°³ïÀ1¤÷‡‹zÀ:ƒcj2£ÁÀ<T^üå™@8²yŠ@5!¬ˆŠ?ÖëU£öiÔ?Üýi¸*~Y@¢0[è^#?údW†¤Ÿ?îpï ´«n?ى+¶c¿æ˜ZRp¿íßø="ßE¿ÑƳãÇ»¿ïÕå¯ò¡sUNASNone?ÞXì›è»t?ÉÝ®•À,³?²,çâ«T?±T:fŸ®?Ýٝž™¶?ɠۄ×Þý?êj­OÃí?À¾³«ß³?°ð.c:0?´°éb¤ïè?»ºhÊG°Š?µî¶WF?å•Q¡žV?®
ç
C?¹¬¿e:?žl(%6t?ÌÔYÆþŸ¢?¨[gsW?âðUöC"0?°øY´P•"?±©óù¬Í?§ D'*õ	?Õµzno?°^6Äý†4FGL J2131.4-1124¿ëîüú‰jðÀDN#c²WÀ:½T#mÃRÀ<aUy¯‡@cD¢œL§@¬Š7&?ÔÃmãæo?Û(mÀÍ»@9?l&™È?ûëg\…'û¿è…–½q:*¿Á¢Ú›¦º¿åÕ<Kv¿ëÙB[Å"´¿ïÿùJYQ?ïÿÚ@RÖgUNASNone?ëë[l6W±?µj¤'eœ?|}D^{w)?w|ú$þ)À?¾ÝPXe‹?´Å›ŽFù?ê›ËgX¶^?À"u^Þ$ë?¥Ð±k—ˆ"?°q5?À¦·D'?¸}ÏHf;š?èxUO"?¬ƒ(YY?³7À¥Ñ‹Ì?˜9¦Î;;?Æ?£ÁûÇ?§Q«±e&?é²d€›ò?®–œàÊ?š…Ò¦šs?'³/À5?Åõ}C?è?¬oòOµžÈ4FGL J2131.6-3714?ïðÌÓµ,ÀG…WÞ
fñÀ;}ÁÅìßÀ<±ËY/F?@!B4éì˜?ÿ "•MÚ~?ÇB$½¤Ä¿¥µË\??âyÆ?"ë_@É͓ò?âh®_ybB¿âoçïhH¿äþîÝî³'¿â¥w=¤%d¿ïáÜÿI÷›?ïÀ­TžéUNASNone?ïÔÓAøì?s?å=¬Z?H\Îi?K1AÇò?rŠÝŠ1æþ?q–â~äËO?ïEi¢?™6Ó¹ý¿D?X"©ÿ¤_D?gќè¾&?›4S7X…Ê?—Àú]¼Ðñ?íכþŒË`?'¿sÉ!"
?mÊÓ#?|ŸéyþÇ?®*þs•#?• ¢ŽÆ‰?ì¸3‡)d?§Ùü *
?uT T'H;?tùŽiœ\?¸é!ÁnW?¨ _§Zړ4FGL J2133.1-6432¿ÛìØn|ÇÀD¤øßzN{À:Œv›gÐÀ<‡Tn^@tG]â‰?þ¡ú@£^>?ÀV9ˆý?äê^x[[p@r)AAé¯@0ì1A?ïü\ý†þâ¿Æ"œY½`ž¿ÕD«@5$O¿çŒ |aû¿ï"®"g³î¿ïÿÔÌuŽøUNASNone3FGL J2133.0-6433?™5#m
)¬?—#ï鎅?îw«ˆÓ¦²?¥Qõ§ì?—Õkx'?˜ô7›‹K¢?¦1½wŠ?¤75t £?ëãß
UaM?´Øûý[̏?µÈ)™hU?°4Ài¯Ö?¤Ì·Mex?'ãä±½\?ë%;Ù8+Q?¥'iUûü?¼oŬò¸?¡®kãX]?«¤¹
¯+Ü?'=ÿZ'õ²?é· o-ÓÍ?­55}M®?Â:PœåÕ?§Ì:œÊ4FGL J2138.9-0408?ë©¡F»ÀC\ó^1
¿À;VÏj5þÀÀ<¬àŸèh4@Š ¹ˆø7?úC(ùôMD?Ý3ۀnÐ?æÁqðdx@Kݞ¬(@]wõ#¿ïÑ
ŸYƒ¿ã•Ð-hï?ïïñʳ¿Ö@›Ñ'>3¿ïü–ä•¿ðUNASNone?ïݶRbþ?uEå±ùw?XŸöQ`Ç%?Zߦ¦ó•Á?eú"ìžÛ?põ4£_u?îm›ôÿÁÖ?«vT¾9?tÔ·Š[ô6?‹=ˆ9{ô
?¦‹©¾¸d?§ùø(]èó?ìOùÄÙ£r?¡ó×8…Ï?E¤cGÓ?ŒË—ÏN½^?¶.ÈÀ`ï«?ŸÄÍÈ$¢?îA‰`Å?˜:¿h*¦?n7:ÉЫH?lËN.) µ?¬hs½VR?—ËwRµïv4FGL J2141.4+0733?嘆˜vUÀ@6*Ã") À:…ì燫À<4ÛE5"7@kTù‹±@:aàŨ?Ãóʨku?°‡D­Y?ä¬é¢Æi?ú|=•âªÛ?ïÿtõubƒ¿Ûh(]lAÈ¿çì;AõmÖ¿æL,ÿ<Œ¿ïÿõEq#?ïÿµøtñDUNASNone?ﯞßüÁ?"Ç™r,Ø?K…8™N?L²¹\ù<?'hëÀvf?ƒÎ[ÞÍ÷_?í¹/p§l?ªßò
u¡3?ƒ.¿.Ü=¢?ŒÝŠy/"ú?¯›}=>yá?§d̽ú?ì›íÎúÚ?›èªEdõ`?•QiU»ðé?…@/ël´³?µÌ72º3
?—G€Æ&;Þ?ì
N{y1d? Åa^év?žÏ¸:/?Œjúteß?·áž¶i?›­²Ó¶L#4FGL J2142.5-2029?îNJ,-`ÀGEŒÒ
ú/À;oA×:åÀ<ŸÒcÃ@ ´í6y¹ª?þñ#Xʜq?ÃN	M[¨¿'á´+ì?Ë2að
?ù\ò3Ž£¿ïÿÒþÀù?ïÿüÚ±'Þ¿áL	Þ¦%¿åÁ(ôëÏÇ¿Ëì쥿Ëiº¸M9UNASNone3FGL J2142.6-2029?ïæ~ÆlÍ?ueO¹Sýk?-(`¯±5¨?-1˯	°?h*û.˜ B?uîՖ]ä?ïg½Ó»?<.ž'›¥?DȪÃÂÊ?S­u¶÷k"?'bFPÒ?Xøꮄ?î")‰KS?ŽRoxWµ?vßÈã€?lÚûâ1oû?«+ÄJûJh?Œ)zôÄ¿?î[¦`Fh?'Yð4XÅ?mƶ¤	?eøOÖYS?¨s/±ÈQ?'Vïª5N4FGL J2143.4+6608c?Ê·ÚËΖ@#¿;ÉêpÀ:üíüÈ=À;¾X0ë@ÀU9@Þ~bÜn+?ÂÌv¦$—d?¹ŠÔø³?ödˆu"ç[@É2Vˆ?åguZ0G¿á~¸+¿ä߯þ_ìпêDùdŒW¿çE˜%%Sw¿ÅaŽ:jßóUNASNone ?ܐ¶¾Ê"Æ?ÄZù"›?ËÏ-³??˜¥²‰8#?áCq^Ð?Ķ—|?Ù?åÐóR=°)?Ç*öÌ6Øf?˜óúª'œ?Ÿ³{ãM?ÒÎÙ°Û~ô?Æ‹C¸ô|?äŽ#&ˆTÛ?±(;£sÀ?§ÈÙþ¬Z?L©7ŽŠ?Óñ —¯€¼?¯FXãçÁ?æ¤-@ƒO? ª¬òÂy?¢Bª(–Iu?‡K*™½Fe?ÐoP9ç,3? r@ŽáÖÈ4FGL J2144.2+7709c?ïýX]'P@2.bÀ;y⏬°ÎÀ=6.Ú²@ #apˆSK@7#û‡Ë;?Õs4?¢­??ïþÑa‡•@òS—VÉ:?÷՜NÕ¦¿ïÿÿ&¦³?ï芘tÖl?ïÿ§ B€-¿Ô:©´™Ð ¿ï€]óÑ"?Ý+%þAcøUNASNone ?ÓV""ª?Ë}˜Üòâ?ß<"T
?Îw°øi{Ž?ËäÙÑØ.˜?ÊXü£
IO?Àü"+nŒ?Æ\ð"»l ?é<<~0È3?Ìé[½Ê¶æ?µè"è"áP?¸=»X02?ÕFïIg8F?µ1O}z&?Ýò¢	—G$?¸%Ánͼ?ɌÝZ-?ª©qwù^ð?À>jdyh?¸a¬ª5ƒ?éÁ¾u
lX?½RXñ›ç?¥ã—T×? $¡G.4FGL J2144.8-1600?ï&)lWcŒÀF¾÷øËÀ;u¬QéØÀ<µ
qs	ã@ ¡¦a(9?ùú¡¡¥×•?ß;m>qÕ°?ÔrcÞ=?ø™&âÂØW?ûZ$¬1̬¿êï<-­¸5¿ë†®Š©<¿×¯•¤—y"¿ç°¹`´JË?ÍYjªmÒ@¿ïÿþR€ÖTUNASNone?ïŽ_È[3?Žo)5!"ê?N¯>æßë?Rò	òýæ£?Š}úÅ<'?Yæÿ(¤'?îƜFôS¾?¥lqXÙÌ?g㥨í;N?v¹êÞt?¢6+ð\?£pé1û<½?ì:k)ùÜÑ?¡ù'ܹn?•0Aª(êx?†hêêþ‡Ù?¸à–E¦Þ×? 
КñUŽ?쥠¼"–?¦cÔoAmf?@O¢¾gSå?H¥ã™MAS?º²ZÕæ€q?¦^µò:¼4FGL J2146.8+4808?ï|¹JJ7À}	@¢CÀ:oD"n¿ÑÀ;È[ז@FE}@¥1Àll:?Ç7ׇ»Ëž¿…ðYfE%Æ?ÁÊTâÛVþ@#J|ù{¿ØɁÿ-½¿Ü@ŸWs¯¿í±VNÁ¿¬Æ¡~Y;¿ì­×^v-?°žª`Í[yUNASNone?Ù#×6?Æ \"
 ?Ša8º_?‡Z¸¯ää?ã
i'{w?ƾ"·çž?æ·ÓøÙ?Åy¬J3ùY?PuÂ3ܞ?cʵ•èï?Òä#Úq??ÅgÉ7p}d?âd˜åî?±ý­´;…p?©ŠI?''"E5ò?Ø<1›¢?±ÄÅj"â?ìÀ'Ó–F? ±«»æEÒ?vï*
QœD?lá	¨C?¸ Ȏ4
? TмFŽ"4FGL J2147.4-3854¿êPêõñxÀI\лnÖÀ;Ij­À<†,9
ä@!ÅX^è@ÈÈ@vÕ?Çãr€¦´¿Ÿåg}+"?ÕXTßd@IqŸŒ¨¿Þ¯¸¿ÏŽH¿ÞØs/Àã¿å!wI¹L¿ìŸÜßi‡ƒ?ÑÜ*7áïýeá±5mUNASNone?îû|_Œ?ý'ðõ?`¬5¢¹¿¾?[ݶ2y2ä?žzù?·6X?|…§Ý'å?ï:lFü?œ~_¹l"?R盽Ÿ­T?l©´ÆJN¯?—ƒýBE²?š˜ƒæ*G?í§¢·cé‹?"ÌÙfϱ ?"s±Rl3æ?xÌ°d§ýÉ?°4t"-*?'»‹	‡¡?ï:Q¿2
¿?"þÈ`¶ê?1¡g`y<î?2ô±Iⓘ?˜oB|<c?"êö ¯4FGL J2147.4-3713?ïÎô9£9ÖÀIðEwÙUÀ;=£_9MÀ<¥°<«'@Jô	Q¸Y@
© öÍ?ÔiÜÓ3?Ç(xY­ñ??ñÅÓé÷ÿ@)T ?ïK¤C@Çp¿á`<ZX¿ß£™!пå¸Úýgr¿ä°?bì^c¿ïÿþó…õUNASNone?ïÛû¸äá?dÜUwR@?AÀhL—ÿ?8åá¢ÇI?o"Ç&Çø{?cx/…ê¦M?ï;쥡¤š?"Lá*žŸ?R>&ÊŽW?aXB¼çÁ?—^ˆß+ç?'fà0Ú¦?î̊À¢?{aßË7?€¿"]ÑV'?rˆ4iŠ©?ªÀŸß B?‰»Þ¹"?îr-a¶ž?ŠÃ~Z^œ?a ¯ûÖ¶ž?Ub?Qlù?§Ëä຾?Š¦eÄgÎ4FGL J2151.2-4034?ÞÑü=ÀI^xB0üøÀ:ó'÷¾èÞÀ<£›€#¦Î@Ö7"¦˜?ýŽ]%u?à.ªØ†>s?ÊÖ¬Š2é?óŽR
}?üɇ5=úb¿é¹j"Ù5?ÑJ?f9¿æ(C ¾¦ï¿Ò<Š?3œ¿ìòs_ž <¿ïîövÛUNASNone?îükº&i=?•ýüy<—?j¯R,òÕ?f;dhãÀº?22Ðí9ò?•=!Ù¯KÅ?ï1eƒÞs#?– ×ŠÒ³?WÝ	˜SF?hXHtPC?˜U~ê¬k¤?"üd—ú¢)?íaLó¦i?˜Œ¥—??á³­ë½›?'à·ÛÈãÍ?°¿¬çÝO?"µ91µ´?5̱é?~r;ß?iMcˁ?lØC¯_Ã!?¤á»M"¸?Ž{|Gã4FGL J2152.0+4718c?ïþƒ7(òÀF¶¿DNÀ9®	SeØ¢À;À*zýÍ @öê5hl¦@
Þp?Á—ZúøY?Àˆb½Þ?ùÅށ*7@ՐÒÇñ?ík»9ýR¿Ý]Õ¾bü¥¿å {jÚin¿è>25r
¿è$SN[®¿âþ_
UNASNone ?ã¥q"äF?¾ÄÖ>{E?'î>Õ ?ä.¨ÍÃÚ?ØÃdÖJ?¾¶*¢³Ê?Þºcß÷rX?Ⱦ´|~¶?ˆºvBþ4y?'$ñyJ¸?à?ä6øN?ÈèHÄú<?ãÅ$Â]›õ?­Ç*±ÿ%?ª鎄¹f?ŽÜ†ÍÆ ±?Õ2ÙIt0é?«@ށ±cÔ?è3°|•G?¡‡;^þß?«Òn†'©?2WêŒâm?È=eœƒÀƒ?ž
á3jÕ{4FGL J2152.5-0607?éhóÆ`ÍÀEP|àP7À:ÎØÿ
6»À<Yÿu6@^X(`t@MYŸ®†'?Áí¤ž/€v¿»¾[T9"?ôáQ¿tè@ ÷TX?ïó×Ûôˆ¿é¾ÃŸ§z®¿é=²GæHŸ¿âçØVmÊß¿ïûDgõ?ïç!ý€É¿UNASNone?ïáÿˆŽ+ƒ?müäQÚy?`Ší‡»a?cG¨a¾à"?[ÿÙ™ƒ–?a…¬<ð?îĎ×Ñ
Ï?¤Œ!le´D?lŒ(CÓ8·?…Eic)к?¡îOþ²?¢
¸ÿu6?í±Búe>?"âýó3n?"ž>h{?w'•	É¿¾?¯ÄNJ

7?'8hՏ?ï'ÁÎÛwÌ?‡f™rs?sûÃý˜>?lä6Qöü…?–Õ%P`s?"'yMˆ¶4FGL J2157.8+7142c¿ï{ ò‹@*˜Þ 3çŽÀ:)öi~HÛÀ;©Â@ÐO@š6ªŒ1@;7T*?Ñs&hI•u?á©ñÖq'=@	ÂzÊÒ?ç¨"õ^¢‰?Ñàu =)¿áx+ŠÈE¿ê7\Wï«¿éò6H'iI¿í"bøóœD¿ïðà<ì™UNASNone ?àhpUü7?ÐIÈe-Òà?ÇJÍIhž–?ÅxØY44?Ӊ¸±¸F?ÉÀ`ÀÔ©?Ï|§_å4ï?Ð?¸îh?àÚéqË?Ó×á_ªÇ»?ͲØîÃ?Ç*!?Ùy¾ô×?¯JeÿxÙN?ÉÙ%µ
?¨cz¯ {4?ٙϵ'¢?¯ÉIøéU?£ÈR»¬Ûu?‡'[Ú%³?Þwµ–¼þ‰?¹Ž™Ñ#ôö?ß@Íf?¹‰øaËÛ4FGL J2159.6-4620?ï&Ò:'¡¸ÀI=žÇÀ:—õL¼À<rÙ	1µ@!)n'E?úN¿ÓÀ?Ãæ[L
?²ÓF¹wÛY?ðî¸Ê·H×@5Ä:, Å?ïç3€`°¿ëõðý®—¿†4›¾¶¿ÒÓ¿ÿ4¿Ý?R[§¿×–ž<–‰DUNASNone?ïŽZUgÝ'?ƒ'í⛄V?7桜ә?/RF
p.H?‹ª5™"`?'ñê¶AW¡?ïXc89?ŠÈ«|Hó"?;Ñéñ)s?MÀ	'Ÿê?‹ËWï2hD?‰ìž%v"5?헵Þ;?—#|Úº2?pF"1?]Wa–zÝ]?²@£níç?–‰ÔuDyæ?îa'Ùd?‰Ñ=Ö?X—	ø«I?Hw†àßÈ9?©(Ê)-´?ˆÛjWÀ64FGL J2201.0-6928?åÁ;ýÁÀD†Š›ÏÔ¿À:"›¯ôOÀ<n¼‡k @ö×?–@Uن³U?ÂD²w$K?×p"[<Ò@1êÝY@t^ÅÞ)?ìh§¾öJu¿áþËí©¼'¿ßÂ^ß´[¿ãßbцoñ¿ïÿü¿ÙŸC¿ïÿà‡êUNASNone3FGL J2200.0-6930?Ûµ"Œ&?Æ6¶À5Iâ?ßüõNI»˜?ÆÿœCe
ø?±7ü¶ªá?¦ö壶?ãRÖØ
O~?Æ	:äA/¦?ÉbìÀ³à`?‡m›3(?ÉQ·ßá¨?º4çY)?Ô缁Ï/?¶è4ږìo?ÝÒñm7??¸'lÂmTÒ?ʊ¤"§ó"?¨}®ï9°?àK<ÍŽÎ?«þÝÁj©j?ÎØ°˜ƒ?­$ƒæ2p™?Ïû	EA½?¨ˆlThg4FGL J2203.3-5009?ïý%¬Ú5ÀIWÒòäÀ:©YÿOÖØÀ<j–gµò@êNÿ—z[@Ï8à^*?ΚÞ=7˜ô?×Õ¬$5¿U@Ê%£'·Õ@¯Lejh¿Þ/]›f£M¿ãØ®¸ϧ¿êu|N/7ü¿îCˆêí¿ïý¶CôK—?è"ËáëBUNASNone1FGL J2204.3-5017?ïۅ/Ë…?¦Ï:Êø?S"¡ê1?Ì?Žþ<?qä?j°ÿ‰Ü?´Ò'Ç~7?îdX'‰w?®Z®ª…Fó?"¿«"!þM?"afKn?ª©Ï˜¾é?¨F‰ë?ìóá­Q?ž$S³.?™<Úº¾?Œ¿-Êúýx?²â|
"×?™,ê´":?îë#ÄøÎF?‰K²üËÈ0?ð%™ ¸?p¾T²ˆ?šŸ`ï#?†€|'q4FGL J2205.0+0943?í
Ôã†^ÀA¯íúCþ]À;ÉvÖöò:À='õ`iÍ@ó{}"»@:a$Þ?Ûù©#Ð>Ç?ìlª]a/@RC;¾òï@ÞÄfKäZ?ïù"ù÷¨¿á'åÞÊm¿Îª9º`äq¿â'N
ˆ¿ð?î)‰¡ÑUNASNone?í<­|?³ÈJ†'[?¤ûãí­j?¬¬†o¥L?§C@ª©?§^À茚?è¸]1¾ýC?ÅeXæå?·Îé›Gþ?¿(0qÛ^'?Á7k`ä?¶Ý‡aâ?æèÇËÈ4?®E&éË.š?Àœ¨æÔH?¤-á_þó?ÃÀ7ê?¤1™o¤?èæae?²Ì¥	õ€?ºÆšUC?«Ÿí´?¾V&̏?ªå¯•.Û­4FGL J2205.8-8254c?ê[ÀçÖnÀ@+L`RPÀ:·ìj÷ÆÀ;ŸÌiiP@Y7žR@Ì}´'m?È.ªb?ªË¡~•\H?àV<'gMí?ø:*¨öü¿ëÿ!HO$+?¾™‹¬Æòî¿ì¨ X6¿ãÚ«'!ü¿ïþ/ ¬ˆ_¿àò«ÿ!Þ¢UNASNone0?ï,ó´«ã?ŸäAS%CË?|À§kúT¸?…"ò >u9?–*7®kîv?›rø\wØ?í<të¼ò?²~C)?˜ÌÎëgæ?›T;¯Â?²i?
¬«{?­|NL	[?ãºG1$\%?°ÓÞ z9n?°¯ÕތHd?˜bøQ|n§?Ô_|&5œ?¯=KD?é"pzM5?«ðÞƬ¦k?¥ŸÎ×`?"Mp]°?ÄFJ"QÞ?©ÆFUËÚ_4FGL J2207.1+2222?©
qñO‡)À:‹…ƒb°À;EL¢pñÀ<¤«ë«µ%@!/A0vëD?üãÙßö?ÌÕl®ì?®4'$D"?äfwŸ@B{pcÀ?ïùß?>¬¿à;×|S7µ¿ß:â
¿ÚG_:":½¿ØA«0šÒ¿äؼßï¿@UNASNone?ï1]–¾ú}?>UÿT1?A§ý½‰?7j"Y"œí?™G
:4dS?1¹"?ïQéêê™Ö?'Âõñ¢V?L|Id£h`?oYråsC?"ÞàW‡©å?'(_k`y?í¬OÀk3)?"åOzô"3?l¾?t¬?Y.™»Xw?±·'ô4k?"P¾'	Ì?íãLê µ?'Ä@
¶fŠ?ZÂƔ±-S?PoÞÀóŠ'?°zÄ5¢?'à¿l.4FGL J2208.4+6443e?ïdþûÚ<³@—Óºý—À8ꈟvRÀ:þNôYÚ@
¹Ø©Nî@ǝZï9ß?«z}þDN?Ê(dM1Œ@)'^aµ'@D¼(?ÏÝ5$Ïî¿ßi<x¬9¿ãjMT¿æ;5`4>¿ìŠþ_kö¿ïÿøsCÄ{UNASNone3FGL J2206.5+6451?ʹMòÖõ?À¤J—Üò?Ü1µŸðB?Éêâÿ–»'?ÖqÈPô•2?Ä-Â(?ëi°j?ÅGmšÈ¢?áMüût}?Ñ%Àq¾?ÓÞ27Ô>Ñ?Ë»_úâ$f?Õ¬ÛÀ)
?³®' ÓR?܈fFï®?µ§˜/==ÿ?˕|OèŽ?«Õ²Kß?Âs 8dÊÒ? ©J='Í?×'ß)!?µyd=ã·H?ߟZ¾qv?·TèÊSpv4FGL J2209.2+3710¿éu÷‹'EÀ.…yRژÀ:¸dàTÀ<D»ñ³6@êkñÕ¥@a
¿cí?Ƕ5?Ìt?Óóm_ÿÄò@õ*Ÿû ?ûãq#®°Ø?ïçz,ìÈ¿æàyó$÷¿ìܸÓÅ¿è]æe$G¿ïéºy
2¿èt¡B‡NUNASNone3FGL J2209.0+3652?ìvh‰yò%?¶gé@¨ü=?³
¿Ôóys?²û|þ~A?¢}÷¾yêÓ?žÂ½ùó7ì?ä!ø¬·€"?ËpöúÂ?Í3ežX?Çøƒê@?ÂEè_V?º€IPT,ø?ã"桯?¯}þÓã}b?À¥ŠîÉ?¡ëªI$²?ÐÎ-e
E=?©¸ð…Z=8?׬hóÕ?­"ёßÇ?׆ȆHs¢?²ÕzHœEÖ?Ñt‹^N˜‰?ªTOHß4FGL J2210.2+5919¿ïü!
@
¶ÿÛíÒÀ9r)=æë\À;íÂÚ@l—ù±\Y@´¯Ÿ•\?Îpc?jy?Ï陌- @Ž_f—äŽ@·ètH&_¿ééÞöšüp?È#Á{4ÿ'¿å×<Èk.¿ëÚß_ ¡á¿äʝþ-B¿ïþé6ßUNASNone3FGL J2210.1+5925?Ý¢¯q"ÌP?ÃïÿÈ· ?Íd™ªDÎ?ÄãpÁJš?ÓܞA¦J?ÄòÉü!ð?‹v¸OÍ?¹¿Ü'BB™?Ì;
_Bh?ÆDDœ¢?äN_ÄR?Æè\4{°¬?Îþ#²^Ã?¨uŒŸz?ŲYªò¥Ù?©ì5õ˜?âÓ਻~Ù?®ãðº˜ð!?Âó'	ò?¡ˆédƞ·?Àn÷W–v?¬ UW‹ø…?ç\ÅgsWç?±7'
â4FGL J2210.2+1624?äî¾ßχÀ?€6†¤ÊOÀ:ë 8ÛêÀ<e¶ü@ôMãÕ@Ñ=?%¯½?ÍFž6€?"i:£ŒY?À+Ëö8+@0w±èDø?êð
¿0W¿ìÿÒ]°¿Þ^úâ3ç8¿ç›Þ¸‡›j¿Ú«žê;r¿ïý©^2»>UNASNone?îΣ)yèD?™–´Ȃ?f€C*ˆ/L?_K\h&5i?¡­É5¸øÕ?˜Ô>÷z‡5?ï¤ÈIН?šŠÍ­¯I|?RwIdói?cElûõys?œò`"m7?™€Ù‹¦î?푸Hoñ?"%àE	u?ƒš—¯R:%?vnÜ·éãÚ?°þêƗ›1?'ûk@0¡?îª^àåD?…3ƒPîz?Ydÿõœiå?L_žvq~Á?¤ŽéñþÛi?"üö&³˜4FGL J2211.9-2924?çb_VãÎÀK|]¥qÀ;X°ô)2À<Ìõ¢®ì@ºò°Œ$?û'SÚr§½?Öã܉Ù2?É_ÃõbÃ?ò¹K{(•J@{ëöD?ïÿ|'1ž?¤Gò\ÿ4~¿è?k*M±¿»	<¿¤¿ä<~`ƒ#¿ä§f pbêUNASNone?ï®ÿF
¢ß?'ß|Wtž¾?Aü5@Û1é?@Î`LÌê{?ƒ k)I"Í?'Žßšééh?ïªnSŒ¥¦?…)õµç1w?4Íޜ¬Ü?Ha&êtŽ?"½ü'ñ/¸?"ˆ5kþ?íì܉ïÝ?'lØWN?wb?þ¦??jN*ã;‰S?®Eïn,:B?V7M=Ô?ïfxhÉ?xhô3éQ?JQ ø…j?C¶ðqåË?'^s÷ŽºË?xpb¾I4FGL J2212.4+0708?îG»Æ??ÀC=lß&k¥À9ù틉5žÀ<'÷‹½8@A•Ò¯`@Äô@¯¹?¿: 8ˆ÷?àÔ=ÿêÜW@ñüLY@DeÀN9I¿é›¸øÚqÑ?Å¢7"/ü¿Þ€Ç%CŽ¿å˜Ôýó¶F¿îŠ4¡È<D¿ïóðÈT˜UNASNone3FGL J2212.5+0703?X5Ó<h?ŒáŠñÖ±e?ï.®£¸t?"ÊÉ+xÖ¨?"üRþ¦©?'s?ŸÄÄ?²nGè1?±^0®ý,Ê?êr(µ Ëà?¾'9¾Ò+e?ºs:†Ï?³Ëåכ?¥9eޓ!?"LAå;Ü?ëÓb
^ž? ÀO—÷6€?¶Ê—<¥Á‡?–зFUè¶?º@›g`?ž²'…ë?åóÌ)p^é?´eÛJ?ˁ¦°ÔT?°þ r³Ô4FGL J2218.5+6822¿í‡¹›}Ü@#"Âß
A1À:ôنïrêÀ<Xu²3ÄS@ È®Õ@
â?þç,yێ1?ÏhMÇ3/Ø?Ï`•ÁóªÝ?û>[ØÉ@Tdù7¿æ9€ô¿ïÕ E…EO?ïÿat¿ãsBí»¿å{:3µ¿âÚ!I%ã¿UNASNone?é±`oê\¬?À0aØBȘ?cú_4¼µ}?cAKÞp¦ý?Èê"Úy?ÀóDÌ´ð?çº>MW×?ʌÚ¯P2?ðlñíR?'øóÝ\>±?ÐÁµ?Éñ¦J5?éé¹×S~?¦A×É2Q?ŒH͐H?z‹ƒ7m…}?Ƙ4ñ­‡?¥SµÛ—–?ë3¼ÜË¡?§"ù®˜?rÿëoÚ?pèA킘ó?™T z?§ek®#ƒ%4FGL J2218.8+4736¿è¤–óՂÜÀ¬'ªÀ:ã5ï¦À<À®	"&¹@©¿©MÂ?ÿDâ–?Ë0‹£Œ·‰?ãæÀhæH@ªèžºjÊ?ÿ½Qӟ¿ëø˞#—	?ï͚R&=¿Óý‰ƒ!7¿âȅufοïUŠáoò?¦M®ß{ûúUNASNone?º#Ó®É?®®ÄÔ¿?ä_ÌÓM2?Å_ˆ€úòÆ?л+ dyé?Âa'‡‡g3?Â/Pþ$3?À€fBæ?ÕrA Jî?Ê6Fdnv²?à»@fؽ?ÌùfßÁã?ÈxOýqÌ?°ÛE­¥?äÃ
ž"/?¶v1ÿ.ú?Çdyˆ=x?§jŒÒ̀?Ûq€;g—A?°›Q)KË?Ú4Hù1?±ÅB¬+¡?Ä´áXžß?£¬,Jpv4FGL J2219.4+3229?́—íá´À4F¸Ø#B$À;r:âTÀ<ªXÆj²ü@!i´6Rø?üÊáö)½i?ҚÂïH£?¿Šk©F_á?òs§Ös?@å"…à¿ïþtDuzÖ?ïõ´bÕ¤?Ý:ÌÏ€¿äTíB83ﻥ°Bi¾¿Ùœ	€²BUNASNone?ï®ÜX®Éu?0ãËJÚ?:g*0Uœ?3ª텓¬?ƒu°'Êö?~ÁXæ¯*>?ï^/"è¶?ŒŠ‡J´?@ŠÐ}å?Y–ÃX
q|?ŠßÓ^Z¨?‹ˆìAÃ?íßT1º¼?Á›üz ?rþ6®¤mV?cÎ姫n[?¯ªöŠæž?*_8ôy?ï»9mû?ˆVEÂÔ
?D³Ö'^ï2?C
.^<v?žÂú­¨V?ˆ
·;ä4FGL J2219.7-6837?Ô&)ØÀEqûçl‹DÀ:ãsê³g¡À=§"ïQ@¶`Ï£–É?øvd«{Cm?ʶI'¼1Ÿ?åU2âUu'@	­Ý|é?ûÚý‡TȄ?Öž 'ðÙ¿ÔÇå</[7¿´•M.±ï¿àµFÓù縿ëљ_â隿ïo)­¯PUNASNone3FGL J2220.6-6833?Ô9ÚP­?Ċæ×Ò?ã*7؏ŒŒ?ƀï&tÕÀ?¶¡]Xå?¯Õ˜wfm½?؃͓ð`?Íåõ!?™}?Úÿ\ƒ_9?Лw1øË?Êîf€?ÁTLz>?Í0ÓHæ??°öùû"8?äõmUþ0?³Óû #Ç?Âtw_!?¢•‹\ek?ã/=hØpž?³(eé¬ö¢?Ï*ð(©b?³3K å³?Ä3ôÛm?£XN9ñ÷4FGL J2220.8+6319?ï´¨+‹Q¶@ßßã*dÀ9Қl'qÀ;%/<-®@` §@~Ú4"\?¿7¢®–*ú?Öík¾?j@»øáþ9?ÿS¢F'^ã?Ó¬îàóË>¿×>l'	Z¿èDîs¿é†ýY¿í'T~1‰:¿ïÿ΁ز´UNASNone3FGL J2221.7+6318?«Ê¿¾(G?£¸¤æÀˆ?ê~øo'ôG?ºh¸ŸK@?¾"ܤdI§?µåZ?•—Ic©Ç9? ¼fPՑb?çîqCeò?ÈàԎ©ž‹?И®‡>—¨?ǦÛcÖå?¼,ÚÆ6¢?£-@?UN?âüæer\?´dԂ(C?Òúü"mw^?°ÿБªma?'™Œ}€??t/T¸9ä?å=·¥Þj?¯ƒ³h‹Íq?Ôjÿ[{û&?®¾1¼X†¬4FGL J2222.1-3907¿àêJê	¶ÀLfѝìåqÀ;»HCe°^À='ÌÍ£Œ@ /ƒ)j²@
­¾Ìf?ϳŔÊ'?"½l˜À¼Ú?É B€-6ð?ó—8¦d®*¿îñù@É?騣ÂèG}¿ê^°Å/Iš¿Ð¨n^,†¿ÑÌ1|#çç¿ïýëóفUNASNone?ïv_ºª?™·<1é+æ?R­_%KRI?ÉEg‹?	2¸hz§?"üy—(‹?ïnì\Y1–?'<[¶ÇP?H5`(SO?X+8¦²šZ?'`˱؊É?v¢jœ÷i?íçËp0}°?'É{G:{ë?xML'OŒ‰?si¬±¾²_?®yŸjÎ3g?'H'QXN_?îžà#Ó؉?+Ëd<}?iQ¶É†b?c!6ãÃ#©?¤|âV*T?Œö¦š#4FGL J2222.9+1507¿ê±ê즦ÀA<fÙ×À;]`—Ì:À<¬ŠLõ|@éd'%ÜÞ?ÿ'ˆ˜ÀUÆ?ßuaù±?µVóרî?Úèpa'ëO?ÿßY´Ò/7¿ë°ýñ‡í¿å'¯Šœ¦"¿ç·ëÿ—û4¿Åóµ™ÕT¿å³ÿvmE¿Õ—®\õ#ƒUNASNone?ï›GüDéé?Ï~Õ?JÆÀ¦+h?‰¦"d(p?‡"äbÏ-?|µ/ Z?îï½~òS-?¢ë^3üzå?T¢«Ž¹«%?h÷£ïC? _´dÿÞ?¢i	˜ë°?î/zÉt?3rv2N?oi†¼ªD?`tÊ6Qª7?«_çž?=D¥Ý?îo·×ֆ?'šÊŠ"Ýð?E‡ïä?F¨4ÒÝ/Ü?¨®bÃ#©?'ˆ— Í4FGL J2223.0+2704?ÃEv™[ӈÀ9£œQÚ¾À;0<{±QFÀ<‰SŒo¬@=:ªËÆ?ü««u+%?àQ>¡{eQ?Û…;=ð?û»'øme@¦NTvÏÀ?ïñªÒ§a¿àç}mi¿à͒?2D÷¿Ýi'z™#R¿ïÿüoQÇs?îû¬ž¯7UNASNone?ïÀNt¾?x®	B"?T'¬ÿ9ô?U;Fü½?z´Z´¯_ß?vQjÁù²?ï!}<
é?ž¡£ï2?E?gU¡‰qÙß?j%ñí}±?œ1'P…?šxõœ£Ÿ«?íqœ<?šìx¥µýÑ?šðUa¶»á?Š¾¿‡Oo?°¸]Å®I?"ª8Jq?îÞy<l—Ô?ŠÒ꽚æ'?JöR1‹h?J¬AåÓî?¡¬'ðpT»?Šáaô4FGL J2225.8-0804?¤âÕ¦ÀITÃóà7
À:Õô_¸Í<À<xÀ²¤-@ z@Ï~?ýæp­E£?ÈëæB"¥?À›Æ…
ƒ?ö×#gäè@ö/ýV'¿ïÿ¤Dî?ïËŽz\¿ÚÞ߉gó.¿Ý6çˆ9õſَÁ#vQÁ¿ãU§11Ñ3UNASNone?ï—ìEžûº?6
TòÑÐ?C²£T'Á?=­7àc,Ð?ˆÉÄb÷õ‹?~y&ðÃ'¡?ï‹m!+~?ˆ¯MÕyô¢?<¾¸"
?L$73&Ó?Œ>Áô¿?‡é2‰;÷?î'úÊf?õv%[SŽ?p,úf²£?Xžl'+?«zÓ?ÃP?ŽŠ^?¡"?î'g'ã%?…à2êý»?f–†bÑ©°?WÑC=Lh?¦p¡¤³%?…¢©@[g4FGL J2227.1+6455¿€ƒ†]€Òa@Õw–9'ÉÀ9ÔyìU(QÀ;FT$D'ç@ß}­Õx@	Zìeˆ?ã…Üî'ÿú?ՀW¾­Ð2@'}ke©¨@¥ºIg}¿ëÓ>€ï)?ïô ~$É
¿é'‡ÂÀð¿ì(ԟÿå(¿Ô$ÀS퓿磢AˆáUNASNone?Ü7Çýw?Æ5G$ó?ÐOÌP,r?È'ëyþ?Óxl¬iÖ?Æb`W"¹Œ?Ïc)+
?ÉC[ѳÖ?ÍGULã?Éú*ëG"?àëeàb6c?Ë1¥n#r?ÒuÉÈ߁?ª‹{©ˆÒû?ÉM }Ä4?°œaVÁ?àqؼ3?°é?H*²P?ל›¦¿¨?Àeê\"R?¹¢¨0å?¹¡¢ëÓ?àýq7¹?ÄäðçË;4FGL J2229.2+6421c?¸"<»Üµ@v2~ØM4À9÷Å&p­À;k3—Ý÷@#Ü­ ¡@Ÿ!Í°"?Í,õ×]?¸'à™³Dæ?ñ`Ñ·Xâ@FŒªó´?ïÉ©—=žÇ¿æbڻοë$Äpù¿Ûg則¿ë¨ø5u¿Ý¨;¾/áUNASNone ?ס{ nA¼?Âþ9x¥[Ã?‹nCD1´3?†]ÙÔÔý?ãÁ‰b¸R?Ã*	?(?Þ: ÊÓMM?ÇJƒN-~)?—ð+'MîV? G¿<×Ñ?à#n>éç?Æ>u3|æ{?áQ'žˆ¡¢?´VHµ)?¨» "ÚF?'~ÓÓó,¬?Ú[Å^êau?³Á2ݪ?ã<Š,2ƒÍ?«ÎçrÑu?¹ñd"3?†tñäˆCŒ?×µ "¯%?«Î¶kâÎ4FGL J2233.3+6530c¿èš+ì(Bû@yw JÃÀ9¸3¡<]À;U¡ZX;*@¹–J@6>Ðö'9?Ä×ñXP?Òc^߉gó@Gª%Øם@ÒÒË>'¿ÕÖA?»VÙ¿áÞó?þѿ檀¥+ô¿ç9¾'‡.]¿ïÿþªJl¿ïÖ¯¤ÚUNASNone$?ÀGE"ž—?±\Œµ("?ƧTv?¹;-¥ÑHl?æfԙ¶z¶?¿‰Ä£Cù7?Ågu™X?Àâz2Ÿ?ÑnÞÉèòÃ?Äj)gmb?áî³VåBˆ?Åև¹¯c/?Ð
èE5…?©¢|^KfÙ?ÆçÙm¦ºç?¥ÁìB
››?â@•có¶ƒ?­äœj8?¾,tÑ:Ò?›òÄ=àðP?ÆHLIôì?¨"o±µ·s?æ¨^S["€?¬l4\Œ)ù4FGL J2234.2-4156¿àU¯Jþ"ÀM2ÃC·õÀ:¡HËJìÀ<ªº€™îS@etùÒ?þ&~3⅜?ÁÛY£ï?¿5£ÐÕ#?ý'ßäÅù@
šZ±ý=®?ïÄÞ˜¯¿ÙÖä¾0&ä¿ÝPd[õP¿Ý_Z©™Â¿ã7PcÅ¢6¿ä©N½þ'äUNASNone?ïæ\õdõè?e²Tk
P?8]§RË?4qˆ»V<?f—U°°µ?d9ðȲSL?ïÅbûɌÓ?€u4ò"uº?*Ôȸ¨¤–?DH `òPb?|wÛÕtQ˜?Џ*œt¯?ï.Û¡tœ?|'-éðÈ,?cƒéslêž?OrãÒæÎY?—ÍG]cÏ/?zçå:ugc?ïŒyQ•×;?p
"k°…?Lý³âGÙ?:ý7ވ±¶?‹Û?Lé?ooçœõº4FGL J2234.8-2610¿¾eÙä"sÀMǝØ'tÀ;~õÒ-_À<óPúÄW@ '®K½@Jv¾£>^?ËJ´C¾ñ˜?'úu7˯}?ÇnÕö— ˜@.$kSŽ¿ÍïßáÒmv¿à1ǂàð¿Â°…ƒâù	¿â$`JmŒ¿ïþÛ"31?ïø'K‰ÁUNASNone?￯0©ln?tîÅ:~ÍÐ?P Üíbb4?I†°èPY?| 0oñ0Á?s"¤!øœ?ïõùŠç?Åªð¯ù?I.㦒?\Ûëg²…?Žr€•¯ ?²(aÏ9m?íªžc°?"ïÜ
}é?Í%¿¤pg?"ÛâQÓ1m?­âÕo°¨ã?d´#ër?î÷ç±óë#?‡M0Çp??Qz¸X%'%?Jê"
NW?Ÿë^<IR?‡/ìøhË4FGL J2236.9+1839¿àµ²üAÀ@æ$Ý/ À;+k¾"üÀ<²³	­'ì@ ¦·ÙÁf?ú»iGÂ6q?ÛGaS.Ô?Շ­¾êŒ?÷æê…Dwÿ@'Q8×·â¿ìÛ;$™<}¿ÔW­Ñ_ſ堕 ãû=¿Ö3ÍA¼¸Ø¿ÝÜæ ]ƒ¿ï÷mõ¦àªUNASNone?ï q·ÙÏÃ?³=YW‡M›?ƒ´ýÂQI?³B¤è%?'J€dß?‹o.meƒx?î[	?Hÿç?ª"?g(?iìYª§³^?~kÊnTÈ?¨°¦pņ\?©?—"ÐŽq?í•4…Ãôü?–"âo¨æñ?†Iüa–?w'»Úz¬£?°E¼Ö?"ó#"X?ë÷Šª^O?¡rmÝ{–?angè	Wq?]ûÙ}Ÿò%?¿¸7mÍ8Ä?¡qʸ&4FGL J2237.2-6726?ïÜXãhgÀFq€AÀ;¼Ì¤‰À<Ó+—]7@ 3M«?ÿŸMR™*?ÏäÄeJ2?¹ü*9?Á")Ǥš@÷Ÿúêü?å).—ÂÿÄ¿âæŽà3·¿âoÒá8ꂿÜ)•»»¿Ú½ÒÉfÿ¿êKWÇýUNASNone?ïÅ#íì%?"'˜OkÔ?4ˆd&‡îÓ?D¦ðE¸N²?|%ƒ5!nX?‹öZ´'ÞO?ï±ïoø›3?'ƒ(×ìE?%òÄyP2?<êÝ¥…|x?ƒ,XñgMï?'+øIž|J?îvˆÓǧl?ŒQ0²v¿?f	!ü}'ä?V³&u¸l?§6ࣽ±?‹]·%ÝAÅ?ï²91Õ
þ?jª2"[wÐ?9"%rûS?-Ìú€Ä"ú?'¥'_+¸?j˸:¾(4FGL J2237.6-5126?ìtMÀ
ˆÀK"DAxpTÀ:ÏfhæÀ<bÜ¢c@kíR@…c¯˜?Ó4Ú–Ž¢?ÙPê°£?ø
e~ßÙð@äÀ»!ª?íÁI̽¿èC}ÎaøC¿ï#¤FÞâ¿àhŸ[zz¿äk¼|±¿ï³¹€iÇÅUNASNone?ïÍUqϑ?ux>W¡¥£?i§Øz~?i§ˆ2Dz?i ²_Ÿ?l©c&V6?ï.YE;?¢ÖrºÑ`?r¶:òYQ?‹ÊuäB§?™Ì­ïšÂN?!5Ř¢?ìÝu•á³¢?žÔoÌA0˜?'e.hiœm?"€+T ¼'?´{¶×ûÑ?›záVœY™?pj­‰?zƒwÝ҈?o_A5í]–?eH
3óÀÃ?‡S—ÙFA?uïª.úÖ4FGL J2240.3-5241¿Æb5m9ÀK[I@»±òÀ9Ç]b±¦À;',kûÒ@ Ã-nÎõ@4M:'£?³ÈJ±ÿì࿦nJáO»ª?õöÁ]-Á@eÎà"j
?áh æ)•%¿ëšJ~©SK?›"*zä¿åYa/ÅÀi¿àÖÔBaúF¿à¡ýì)‰fUNASNone?êþœã'?»…ݲÍD"?oøз"?s©ùRÉæ:?Å©0‡q;?»Puk©UÛ?ï'³ýƒîn?¡,Œ½û'?_´efú¢þ?xú9Æ»Àú?™9ùˆ?Åq P™Ç?èÁX
1è?±u±!.¨b?Ž4ØDž?|˜øËZ?Ë^m«ç'?°ªBJ	©?äµ<N1?¯<w°?V ?zàzcŽ+­?qN/»oAŸ?×rT«ù*ð?¯NRE4FGL J2241.2+4303?¹&ú¬{À+dî
öÀ;µ^>JÀ<Ô6>@lf EoÌ@øBf¬ÝC?Õ5¯D%ɾ?ïÿÜ>Y×ã@R%1ðÃ?æ -Š&ßé¿êŒëÖ}O·?k`ñ²_¿áæ͓œ*¿ït¸¤ Ü¿ïñÓíR~R?á 1ί%UNASNone?éuÔžú?ȅÓ÷,¼½?½YÅpªÌ?Á«p=Ðk?¶÷"¿šÍc?»ù°\~?Åt[€z?Ë:vÍ9?ç:*‡Dò?ÐÃÕò9-^?¼Ã×w?¾fœãá?ÔB±¥[á£?±÷¥ƒ‹ÌE?Ù«°ÇžOò?³I—+>	¢?ҝ"Îj?¯¥×¯?—ö¨t6àç?‰¡…ÿ&@?푕±Î¨?£~4U'}z?ªëYÚÇ¥?Ÿ]Äa|4FGL J2241.4-8327?æÀôž;ُÀ@J^	}À:°Ù(û¡ÌÀ<…Ål†;@ýTÔî"?ÿ‡7|n¨?Êd_:£?ÛÍó}抹@Ê%ïúÏ@n½:2«Ï¿ëY@¹À¿Åù'¾8ß¿ÝÔ>{eÑì¿Þ²	Ò癿îåvå¿ï裝SqUNASNone3FGL J2237.5-8326?ç/cñ¶íÎ?¾Ýqmݺ?ÁêJþt0?¶Ûå¥r-?ÁX&1%ԙ?³çâäJ^Ê?ê±Ê²ûj?¿ñ¼á¶?¬E©Kù½?²·g²,|?¼NÕÉœÑ?²Æ½MöAW?å8Ȉ/·á?´W~]ƒ?ÊCÇhó?²Lã
B£?ÀÙÆØ-\?¡ÒošY ?êtLô©?¢>³i=X?«dÕ$÷?"b-™{Ö|?¾«-ÜÐè9?ž©˜	
›y4FGL J2245.8-4148¿ïù⡗·9ÀN=þ!ÙnœÀ;"E	Œ³À<ïð‹î¶,@"Y‡°¸ð?þ'Ù--_µ?ÓJ"ä(3%?Ï8ùÜ$ƒ˜?÷çESÇ'q@_Î$1?Ò¬cû¿äì¶wò¿¾'¡T£ñ¿å}Ä@âl¿á°'¿ŠÄë¿ïøž;ê½UNASNone?îTOçç
?ÀlÈQÆì¬?"`,z?³´xRÝ©?¥¢öyʀ´?ºú'ãG\€?ï'´/w(?Ÿ…ª¼¡I?e@ (éÀ%?v5iÉAƒh?›…Åtóã?œ	|7Ø,?íB´'­.`?—´¬‡¯Õ?ŽOõù²É?1™'ÿ?² zÓ×Vª?"×	
â?옱ué3R?ÙM,P?p{Œ˜O"?e`}'ÌX?º2»‡6`z?ÏýÍU"4FGL J2247.7-5857?±G™­Ì¾ÀIÔÖõD»À:Ñ×ÙôÓÀ<&0ì1@£Ð3ç¹@¶½2%?½5 á6'7¿¯©¬â Æõ?ñ7jК¸@"'[d±?ïüL·h·y¿èMW¡§…¿éHÆÆ"¿àMÉåX4¿éóaáòN¿ïÿ-½R†`UNASNone?ï/ø)ñ?´Wéºû?‰"¼e×?²‡¾0ÊvA?Š¬ ,è?¢ê
Yü?ïF%©FòŠ?'ØÌF?P&µâœ?\¾±6³/¹?–8ê‹ÑP§?'{×,Íù?î¤ZŽ÷?–¼í¯7t?{™G@…?kO²Þ§e?ªÂ'|w(?Ž/bײæR?îÓ$#8"¬?"3m¿F†?y=›êWIð?g¨òÛ@Vg?ŸLžY˜?'´a5?8K4FGL J2249.4+6222¿émœ µÎ@C±Ã\
ÃÀ9±úã`	À;ü}"€U@;ڌ(õ@¬{­?ÓÈD½IL$?ÇÉD6¶Ë?þzŽÜ§5d?á>ÚJ± –?ï­Ê¾­	¿Ü3Յ2à¿ëÝü›Çq¿æT7ûr¿ì©c`Íu>¿ïöQ*"ÿUNASNone?ݨktVþž?Èé
wæÅ?Èjc¡©?Ãèƒþa
U?Ö"b»z?Èn>ÌHýì?¿ÁÞó:??w$×Î?͸ֶûí?˪ôÕ…o?䙨֟ÙÃ?ÌÈÓ'Ñù°?Ò,—<#ÁË?¬˜)èq?•¿'í$?¥|*aGÐ?âdÎò
cÒ?¯pG^ÒÏ?™•­D¼Å?€¨ÕŒ¯+?ÌY$§jo?´Öè6'Çš?è!*(»5þ?´¬«€\4FGL J2250.5+3305?ʬ¬h~DÀ7H`RP/À:<GËp¬;À<cþcGÍõ@cá4¸ÄW@ϑE7A¶?ÂBˁž%E?ãóÞ>d>Ä@f<ù…'@çâû{9?ÙZ…<ji€¿'Š;¾Ù*d¿âÖV¹J9¿ë²'LÃýñ¿ïÿd™ÝŒ8¿ÞBÛ\\¢BUNASNone3FGL J2250.6+3308?¢'盵=?œ,†«nŸ?í É0·¸?°fóz[\?«qXèÉT?¨K'".{?¹BHÚx¬?¶\­¼ù¾?鞟~Ô3b?¿˜TG€Æ'?¹ÉÀƒì??²3σ/ H?ºža˜Û?¡lŽ¤¶m?çQ^lsW?®n¦<Z$Å?Å®7FIf5?¦îkÝƒ'?ÀxÇÎ÷6}?žàí<&;‹?å—#D/¿Ó?°‰@Íû°?É*« IÊ9?§Ž,wvÁ4FGL J2250.6+5809?èé/ÑKY¿ðûx–ê'°À:§¢>ƒÉNÀ<	ɓ\i@!'8úóPÅ?õM
À¿?ß}~á‡o?ÝÏ`cò@I][û©Y?óüûhÁŠy?íÝ®ˆ*Ü¿ïù¦êºô]?îVÃ[4=¿Ü«›úœê¿Û1s?'½¿ïã¡ìõ6UNASNone?ÚàÕ¥Iâ/?Ë4xqôÝæ?ˆØAZ<?‰o^QC??â,4'ò¢?Ë(g§à¥?Ì~ÆÛ¸Æ?Çq0±Hñ?8+Ü`C?'prŒ®?è¢HqY?ÆØld™Á[?ã`ۓ,CW?°p…Ç#÷?°œˆÅ&éÇ?–çßwIød?Õ&¨]¾ß?­ƒ>°z?Ø&•7EU\?½&Ia‰?êbQÿ{?…ŸŠZ¿F?ã¥ÛWc?½¼ÆT¡ý4FGL J2255.4-3252?íõ¹>X3ÀP"ÊÕ{ÈÀ:ÎCr‰ŠÀ<¤é½ž[ @ÙIŠ8@¡ƒræ§?ÐYkáÐj?ЂƒÓ^·E?þV'Tà@ÙE¡Iç*¿ãÅâB)ñ¿Î	{(ë1¿â­×>?׿æì¶!9¶…¿ê`üßåy¿ïÌvÀü‰ÿUNASNone?îm¶?¢yV£*?oÝÂÔÐ!?ge¡ß^l?§<ÈHpºí?¡~ڃk?¢?ïs|2†H?'¤N/Óa?Q²E…¢Ç?aìÚAå}?uUVäê¹?'ƒF?íÙlՉh?šß¡%˜³?˜ˆ"R÷?‡î‰ g×?±×
Qîßý?"s§–?ï7czöÙ?}6¬*‡†?hùÊ?¬?X< q™5?–"â?{çSgŽ,ÿ4FGL J2256.5+6212c¿ïÿ2|V@ "S.{>À9r« ªšÀ:íև`±ñ@R°ŽES@Äg£}?ÐD~Ÿ˜6B?Þ¸AíHm@[輜$?ñÌGVUÍ¿æmE}¸'ƒ¿«iü"0·ê¿æÔS©Ë@¿íüŠ_iòã¿é!	?nÕÌ?Åáœ}#Â'UNASNone2FGL J2257.5+6222c(?ĘHÆ«?Ä¿šEKà ?¸á"þ™°Ó?½ÒŽ×óÅ?ç½Õ`˜;?Ê"Èçö©?¿Õå95³b?ÃCÏAÙ՚?ÑE‰ïÆ¢%?ÍKºD½Š¶?ãb~`õø?Î~gE@?È/¦†¹?¥2+s®Xé?ÇÜ÷ãF0?«"kðxp?ävŒÅ»?° Þã§é?œpýb‡Ö?†s×fþű?Çd`'È-½?±ø"U{ã?éF<SbàR?³Ýo]¤ü4FGL J2303.9+5554?ÃðèC
­ÀàÒ=OèÀ:Åc®ünÀ<^UªV€@!¸_õ‰Ÿ?üŠ"C"?ÈÁêAÞG?Åq!Àŧ?ü£mWò/@]Ñ8Â>¿ïÿø]ˆò¿¼ÙÃUU?ïÿÎÿYg¿Í7IWâ¿þ¿éÈ}ýܺ+?ÂJÆüÔ'UNASNone3FGL J2303.7+5555?ç`å1¯ù? ­»HIÈ?sÚ´AÚqõ?oóÙC• v?ÑyÓd•6G?Áÿ'%mrD?à'賐é?É0#<ԙ™?k9\4¹%?~?+	>v‹?Þ¥»à­"º?ÉÞû1›?èÒ°4_ö?§sßà¢@§?"P¼
½7?'0ä1æ¬Ê?Ê*ó¬Èƒ?¦ôöìt?ê-øÏ,
?¨.½;6¾)?"s-&fZj?z5^6äP?Ĺºö"‹?§9fÓDþ4FGL J2304.0+5406e?è²R=h|ÀXàkæÀ8›Òß5…À:äk篧"@#7›!Ùï?ü-SaÅ?µpb=·Æ€?Ï>;¤ò@"è‹+B?þ§mrU¿ïÿêњ'ç?ïÿ› 'V‡¿ÜÐæ7
¿ºWìPӿفà•V"¿»?#@÷ÁîUNASNone3FGL J2309.0+5428?Õ£ÑÃ%z¡?Ʋm·6X?²&	ûö¢ª?°	†,›(7?âéUÞînZ?ȗŽYŋ£?Æjòú	1?ÉŒ
ÑÑÿ?Í>†Â¹+?Ð	Å+=¯D?ã¡š
©?Ðb<åä?ÐÚv›0ü?°g
'Lw?ºä—N¹—}?¡ìT^wƒž?ä61ȐO?²G¿D$Ó?­:=ù#Ó¸?"ñ"R@=?çpcØù?³mŽù× ?éB€T̆?³'8(¶$4FGL J2306.6+0940¿ïÌU&´0ÀF£sÀÁüÀ;)Î悀xÀ<†\<@øï@2gà9@‹ƒVa6?Ë'4!o¼P?¨U:Þ¼þ?Û%l 9±R?û:µÃ›Ë£?îêI¥Ò?ê©érõÁ¿égÃd™¿ãôJ?>YW¿ßJDÝ)¼<¿ïÿ!ž5_³UNASNone?蓮k?•¸ä¤1v?a-½%?[|L¿q?›ú…‰ˆ?"­ãÔVþ¦?î»KƒnæJ? ¨DµÝ?fH¶Ò'f?sâ$³lTú?¢æ¼`xö?Ÿ+O-þ©?ízKþ4‡?"·ˆ«?‡Öö¨?wriÉU~?°³ÁJæ¶?'–ê(g,?ìÞ̇jê?š'¸úøßÝ?ŠxsÿŠ?s?ͨ
?µÈŒÆ^(¾?˜³c+'H4FGL J2311.6-4427?ᆲª‡AlÀOǛÜiøÂÀ;@­
ê¤NÀ<¨¯3+¦@TjX¹T @9×wJº8?Ô.]¶i‰?¼¸—
ÉÅ?éŽ_tÝÛ@¶ø¥Ò?âØ"ð½¿é³hb?_¿år¡L$œ¿ÝTŸÿå(
¿åly¥ÞKz¿ðUNASNone?ïà±åºIÏ?m¦ÚÝX?4ÄJ<´J?-:c~°u?lµ'nš?láá|"²?ïv­("?Íß}Y!q?JêB&§øå?Y –Þ¯žÈ?e-9%»ú?cL7"Y?îJÏý?‹vÖÉ8?t×P{ïRå?cüÞ¡rcô?¨Äõ'E"?ˆáŠ§¬Á)?î"èb}ã«?Š•øחÏG?`·¸SŠ¤?SúÓ¥7O?¥¦	œœŒ¦?Š—Åç*Åd4FGL J2312.4+8253?íÀv£S	p@4£ èBtÀ:œZxòZ%À<EÇwù5á@̎²µÊR@½aÀxi?Ð6>"þ?Ôq³/lÕ@ã
ù½Æ @77F¾*s?î8Çâ'@¸¿ãÚ¨ÝÚ;J¿êšÂ
¬¿íÚ)vñÎå¿ïÉ4â_Ü	¿é8âií¤UNASNone?í¬h«ý‡Ë?«ÎÙñ!'?"Ô#²"ð?•˜ûv»Në?ªÏcfÝH?¦âÊ8"ÐU?èY$ Œ?ÄR1ýÒ?¿$œ†x­c?ÀXjû
}?À\M*C7?´úd§	?è[ùi¶i?ªÑm°žG]?´¦
Ž?™a:Öìñ?ҊGR_?¤Ç‹ÜnÞ?ç¹°÷õ=?¦Þí
Ę=?½ã9}ÿð?¢ÓEÉ—?ÂUŸa+?žÜ(p›¸{4FGL J2313.4+5947¿âù	1¾$O¿è«ûèCKÀ:&†ZøtÀ;;ÌÛ…¯@ ³˜zµ¨Ä@‰~Jˆº?ƣ歰¿£$"3ÿ
?ÞÑ0ÿÒ2½?úî5r} ë?ïô`Å<µ"¿Þ• c!ãU¿è_øù{¿ç\¦>m£ò¿Ó4˜Žß#¿ë
Οµ½gUNASNone?«éNn€l?¡‹{÷׎?bd\k]?b#Ê÷sOË?î/h	³¡¾?¡ÕÇG´ÿÖ?ºí€~s¢?¹ÔîÃݹ&?|"û 2ú?js.vƒ?ìi'ùñdÆ?º"o#ò¯?Ò¬Z((Ô?¬C³‹™Ñ6?©²úßb?Œ›ëÔP?å')=¡?«mwÁ¹ã?Âl{±–¢Û?¦·ú§;â?'5M§}¶?yÀË†Û…?ëß¹S?§1CZñ¾4FGL J2316.7-3144¿ÛîØ{è¿ÙÀQ;27Š°ÉÀ;=•ôÉkÀ<Â"<jêZ@èák•O]@9þ¡[.û?Æ%]‡š"•¿±=èîÁi?è¹EÁ€=}?úˆÂ>SwÌ¿ãýž%ðU¿ì´R¿Ýñ¥U¿ßgk1|¿çŠ¢OοÕð?ÃdnUNASNone?îÑÞÒCN˜?Ð¢û,õ=?_Šª£²?UÆ&-^f˜?¡å¾Vuýã?M§‡¼N
?ï`]T[l$?"ƒÈÛÿ?R·ŽÃd‡º?b
gâ?/?'È܈\2ú?'Qú¥Þ²`?íôª½¶Tt?ô½Ã$é'?Ȫ>8?v|º¯Þ§7?¬¼>ÜÓµž?ŽhËSÅ4?î1H?º±¡Ý?hN'[/ÉË?]BT5¹?¤©EG8'¢?Œ[¼'3|4FGL J2316.8-2518?ßwH"ÕÀQ/Ë>WS¤À;j@ºˆÀ<È)ösD@8bè,¤¤@7^nÔÊ@»·Þþþx?·Ç¡á^T@r»3rH¿ïûƒ¶?ߙС½6¿Ýåâþ"P¿åÏ\>oQr¿ïþ9 ²ýï?ïøª O€ÇUNASNone?ïÀâòY^g?˜WDZ9çû?nÅ°~ø?—νÊg§U?p+øûP?péñNÞÓÊ?ï†ïØÄ?•ùpD-¨?UÛÃÒrùô?tûuà­-P?‹ˆ'…qoË?'©ëë00ñ?í«»HÎr?š	IÛü?"Ò:ÁÍ/?‰¿ysö†â?±ÎuxÙ#?"ù§±šQJ?ï³ ¦?£¾r‡ïLé?QŸœO?T«"¸¯¤m?ƒ˜'Xžu?£¤ß·˜4FGL J2317.7+2839?Ð1…Üß{À=ÜÏ|ªuŠÀ:j‰á•²À<hÇåÝ?@ [¡äì©6@'U»Gi?¹nlŒñ¿—E`dø0?àšf³"?ã@
Rí*eYK¿Õ·¼]éÀ¿ßôYĚ̿âa8ÿûοá+8'ŽºC¿ÞÇ¢@‡.³¿Ó\åGB	UNASNone?ïÚ«G8X?g0Z*«l¥?5»¹s`JÜ?)?LØ"ùç?qN Û-Ïj?fCrŽÇä8?ï²='#°º?'Ì"<$?'|âMÛ??Ç¥e^}í?ƒ¨.ºœÆ?'dn°'?£?ï3¿¶^¤?}¶S̲ké?_b'ŸL)?Oôv&ƒf?—Ž3³öÙ?|¶TòŠ»Û?ïVªñóu?xì	‹©¦ÿ?JýGž!Á?<
Öï"Ð?"R·"­ƒO?yN-´Î4FGL J2317.8+6140c?à›ø£.1°?é˜c8´|tÀ:݉³r‰À;"•µŠé@"»ï¯Ð¾@Gz>Š?ÉÍ$`‡;?׺šÛŽ½@
À?`h?ôΨB¿ê½˜]ƒ¿±dS爺ϿÚÈ2¾ïŸ¿éÖð¸»¿é€Å§J¿ïÿþÐñUNASNone!?µBI)¶Ã?«çCÛÝaý?±J²3/óŽ?­×¢óÄ7?ë.`"h
¶?¶àhE'€»?¨žäÜÓε?ªÃÖ<%?·…'Xû¨¨?·x|d»Gï?ë…lÇN?»õtºÑ?È/µnϘ?¥*^Zk#–?ÃY-/!3?¡&îEÄ?åÇXƒØò?ª£4'¤ã›?º
aQQË?–æ'lCEð?Ѷâ™À?°œ E;hÞ?ä.CBˆõ¾?°º›]©4FGL J2318.6-3827?Éh¨Ü"ÐhÀPâpdìé£À;٘áõ²À=Jb¹3@û‹¨jAè?ÿ@[ŠjQ­?Ø9Å^?ì¢E¥%¾Ö@šð{þ~ @Ñʽf'¿ïÿå=†ô&¿ÁPɆœ;à?ïú՞­«¿Þ$#á0±ú¿ìgs¬ ›¿ïý_ÂvíUNASNone3FGL J2318.6-3829?íÖb³?¾¡"K¡†?•õܵ²?—l(¤?±ƒÕë'?z?½ƒ:òÃ?ìø]ð?½ÌP"º(?Ÿ.ÜkáÆ?±¸~ôõ0	?°qmo ?³‰·¹·ð?éÑ«ÜêïA?ªŒÌì§?±
š(-?šF…NÛ¼?À2ƒEÀ,q?¤ßø.üC?ìêþå/?©â"Ä&q	?¨˜`:R©?¢^§¸ÁÃ?®hïלšZ?¡G-nɲ4FGL J2318.9+4151¿ÉbᒒÐcÀ1ŃùdoÀ;¿¦sœ°À<Ví½\ì@Ô¥Èüލ@™#²?ɖ÷¨Ãƒ"?®%{·?åcä
Öó—?þàUÓq+¼¿ïƒ"4?ïÅ(ÉL匿é$É®4[Q¿á@$³=¯Ž¿ëù—eâ²è?±qj{sé²UNASNone?î‡+wmš?¹>47—B?vK¯²êË?q+֗Œœ"?¤ÃÒ¦0¼?›÷¨x'œ?îîÑ`k…?B®ÒK?gZ/6W?¡?zÐ>ž?Ÿ:™m'§m?šl‰.B²?ìʑ¹Uï?œwÊ	ۘ7?ëžN¯ý?¼­'œ¨¸?µpŠ¡¤Á}?˜kìñ›y¥?ííK®c7?•ñï³Ù…´?Ápå"?|9JÂêŽÆ?³Ðsp3Ê?"Y›ËšÇ4FGL J2320.1-2440¿ï똛S_ÀQV灃ùÀ;75c'À<°Ô8í‡@"·ç7‡@'`}Y"?Áƒúuý]8¿µ)žŸgäÁ?óÁC|V'´@mÀÐj;2?æêŒÑ4;¿èÏ_žÌ'¿æ·Î8Ø¿åù˜¨)?µáVáRÈ¿ïÿÈb±UNASNone?ïoˆCÇ)M?Ž'5#?eÁxLìT?aðž{¬Z?Ž­úú—á?Œ¨éËi›æ?ïc	r.Â??šòþ7äûw?Uð̐·2?uY¹änÆ?'?ÏÍ^¬¯?—{;÷¹ p?í©r˜_E'?"›Ð¦_Òï?zµ9ÞKƒ?iÑÿâÛã?±	ygò?"ž'CDÖ?î¨`FLÓ9?'oLU3n?MÜkßô¤=?M?4t56?¥‰ë²ùÞ?'Zɘsµ÷4FGL J2320.2+0707?ÜæîlÀH _ZÙjjÀ;=®¸å;À<‰é'9Y@!
/ÿL%ó?ü¸âe+Ô?ÓÔR?´J*ñpE7?ãà÷?ò=æ*þ¿ìjœ&@‡?ïw·ÒiÅ¿Û~ž¡@W¿à؆¿L[£¿ÃÏ¥ïa¿ä­rÊ!÷¢UNASNone?ïdzeì¡2?ež<•í÷?>¼ŠÐOCÉ?D1U¶Ü¢±?'õÁ*œ±?$ÙO…'?ïFà3G?˜,£2Ü?X>èïÁÒ6?dk«P²êÆ?›³5j›?–öÏXI]?íð<)*‡?'KW2ok?sžE±æD"?l'CÖk?®ˆug0Žò?Í8gÏ?ë"<ã&{?£@ªö?q°^;ªrf?m_TQ)?Á"0–"?£jT1_t4FGL J2321.9-4842¿ìvˆ&CzmÀO+Ê! áøÀ;'^±ŽÀ<™Dwÿ@ð³¿Õ˜?ÿÁ†}]"ñ?Ð
,8m.Ø?ºxîÍ?é¬ÖÝÇÆÔ@?X£Q?҇±d¼m.¿äÛ£ß¿ßfÙRí¿àìÒü'¶v¿â-«¿‹ñ¿íù> #ÌcUNASNone?ï=«}
½Û?‰ÄÜG¾úÄ?P¦€ò%?F×Äu¸?—@(\¹$n?‰;J:½&:?ïoâ#À?'Yyì=ó?K'>Ó@œ?ZO³ú¶Åè?'1s1'bº?"°¸?‡|?î"QÛ`£f?Œ‰Ðð?q­7ƒÕ?_²Í=YF?«¥;i¥Nï?‹
˄~dú?í³ßõšb?"…ºól?aÀK_pÇ?SfàØiô†?±ß*ýø1g?"£¸\ú`ð4FGL J2323.1+2040¿æ™»}oÀBÑ|o½'=À:ÚýPùØÀ<kymª'†@¯ˆc'Iê@¥ÆÁ#?ÃõB6Ü5 ¿¢ðš1o
Õ?ádðD¡?ÿº°?£Y¿è7Ïᗊ¿Ú5ÅaŸ¿ç<lݣߙ¿áʓÒ}'¿Øx\2/ýõ¿çÝu&Ê;UNASNone?îs¬Y#šÅ?žÇÙ`mè5?c,^OÐ?VÓÆØØ?§'tˆÎC³?ž2þÌß)Ü?îçæð¡>9?£ÜL^4F?R'¤0HÏ?aÀ'×ìº? í`ʚ1?£'Ç{˜ù˜?í¨ÚHC^?"yIJ‡]t?€ÅC5 ¬¶?pJGYw;þ?° …Y!Ïr?'¿×yA?î)…c¶$?Ž'¸¥^Ì?djÛcKå
?Wú–ðÝæ®?¬ üiL?Ž}Ž°³"4FGL J2323.9+2519?Ä!rÇÙÚ
À@ºç¯·éÀ:Ï'`—À<‡ô9rè@¢@ÕXå?üqišÐ?àÆdÓ¿/?ڒòK—
?ü¸ŸÔF=Ò?õÑ-=û¹¿èz9¢õ¿äYÈ]ÒC.¿ãEgéel¿Úü•½Aœ¿ê¦k93þ4¿ïýwƒ–"UNASNone3FGL J2323.7+2523?î%:ԕÝ?¢N;SOFª?x-õb?|?åü^÷ã?«­jÌ÷õð?¡œ<lÌrn?ì¦;Bç?´WlŒ»	z?ó:®?—Ÿ)¦6"_?¶Æé*¸Ó?±¯~xö¬?ëQhUb1-?£ÐĝU~'?¥-Ú0«?'y±%‰¿?ºÝÐ<˜î
?Êaxâž?éæIìòë7?«mÁË!ò?Œƒý"]xç?/«ˆn'?ƞ˜z{–?©ÛM¼Ñä4FGL J2323.9+6219?ïÀƒ¸?ò"cښë©À:}Ñs$ºÊÀ;™®°'k@!!|o?@«j©Ø¬?ÖÙ¶Ÿä·O?µta%߸?ßÒèûV¢ú@®6Ñ?ïýä×Û¿î/¬*•ÕÀ¿È†ëA,¿ßu§·iŽ9¿â†=œBÁ¿àÄ(ï'µUNASNone?Õ¤g'Ó?Å0,æ?YŒ·)UR?WhÞÁ«ºY?å!87Œn?Å|ÃþMy?Ìi$Ÿ…Î?Ç>î(?òA?~ۙy^j+?"œÉʘÍ/?è§ÿ¥+Ϫ?ÇD{øÝqÝ?ݦwy-¶?±]Ěº"ç?¢1ÜÀö~Ù?ˆS²(å?àPø47?°ÀºÅØwV?Þo"!œª?²¿Dî?x…w\íM°?qzãX?à—35W?²\ooI4FGL J2324.6+3115?ÂÈ[Ó)LÀ<^ê–À:r®8(eÀ;÷|Gy;U@=eP@¿R%fÁÖ?Л™ðË/?ÒSû)×iß?ýu©dè·å@	Ñq§"=?íïMËdíÀ¿ãƒ!ˆZ¿êªó^1
¿¿îBÜ¢¨6¿ð?ïÿ~‹¡3UNASNone?ïö[5ٝ¾?U'ézã"?A×í!SóÏ?F½ŽõRK?D»;x5Ý?KACp(ú?î:
ŽD/?®«ç¬]Té?ƒ&p»"<K?"Átó
þm?ªrÂø:®?¨æ¤Ž)—¼?ì»ÅR¹z?ž¯lñIA?™2¼"¾ÞÑ?ŠqwD­º¼?³Õ&fê|y?˜Zê+Ü7?î9ªjÿhD?'–Ú54¦Ì?y5ÃÛç?hLó"S7?©B×IQP?'yýŠ&Z4FGL J2326.5+8555c¿×n'×E²Î@7Q¨½#žÀ:²š'^À<1¸£J"@Ä5Õyï…@Vü9¡â?Ìu‹‡ÞY?—½"]?Ǥô^@LÓ±Ã\?n'§¯S¿éTký@¿é'^ÿê±d¿è›ÿ/p0¿ïÿ^Ê¾?ïõl=ÀÕÉUNASNone ?ï˒ZºÄ£?tw©Õ¤û1?eBÀ^Þ?d¤ˆ͐¦?o*äç4~ ?lüü$Ððd?îô¹ç´5Á? NzÀ.?mEÜ4žgº?~¹'˜t?À'å{?œ%BLvõ|?í?¡-¦|"?—©ãÆèi?‰ø)ô3IÒ?z"‰2]Ë?²ÃñTE²-?"}]ëIà?ïk=æ§Ñ?W—>fdµ?_$öç5›7?Q"5ñò.a?«ÈÔ·¬:?}kuþY4FGL J2326.9-4130¿âê'æ›ÀPàñ€
À:h8:Ùð¢À<À>-b@D³'>0'@A–EQBé?Áy}Yò吿™hüe85s?ÒӌDÐ@¹fM¼ÌO¿êƒ
€òç¿ãz–~ÜÿË¿éI‰¶Í‡¿åç¼r¶¿ëÈorŒ¿ïÿûbâMhUNASNone3FGL J2327.2-4130?ïåÿ\Ép^?cU‰–Áì?Sì\y½)?PÃt€ÄÔ?`
tîÒÂÛ?]­KI=v?өȾ?‹dC÷o?A^B,Þæ$?UÎl.‰œ·?†Á&ò¿áù?Š>ˆÑÄ?îäè«^&Q?Š±ª#Û¯²?sL©Ä-p?kOlI(îX?ž¹éÊ*"?ˆ*iñMÁ?ï'Û¿!õ?ï™que?Y7c=×?Kí-øiê«?™r"¢»( ?"'""&®4FGL J2328.0-2557?î	"õÖåÀQÕ_þmXÉÀ;V"tnÀ<撐Ü\@+È%Eá?þQ¶á¨üä?Û¾ó'ªi?ÐSX!+¯?õF‡nêÍ@v>Ôüò¿íº¸˜baõ?ïŒ<"Í¿åCá9Ñ]¿ÃžÅR…¿éñk}&œL¿ïøVž`3UNASNone?ïá@EŒ'…?gÌÎ75e?J'/ãÑÌ?Eu·¿úù?hnzy:˜?dË¡1"€—?﹍©í9º?…0x¥t?5¨µá¡å?KhÜi¥Ø‡?€ðˆ?"\?"ID	ÂZ]?íò#wÉeÌ?'šylúë/?…ñ›PL?yÞ*¬"à?«ae©0?þ3dj}Ÿ?ï—L`\?té!Äáð?Nà߸	èü?J™ëžô¼M?ˆLì{Êh?tm¡«p
4FGL J2328.2-4422¿ä‹V	÷ÑÀP€^"ð•À;£Ÿ}ß(ðÀ<ôy2?@ mnžÄ%ß?ü4 ½¨?×?(ßÈ'!?ÃCºió¹¡?ä{PÙ6h?üZËE8Ch?ìH‹¿¼C¿î:a?µøu¿Ïßü?Eö¿ÊrÜ@ˆ0¿æršA4Rÿ֓V¿)vUNASNone?ïLƒ70v?¢ÃäOz?aÏl÷®? "ÙŒëé?"5¸lRM9?"DB;(hÍ?ïZèN÷¤n?•8}hä?Tn:¢Ï–?e+ًÔ#ñ?"\€ÁEY?"̬3ä¥?íüÏÛº?C¡Ëž6?rˆŠE.Î?fk9;Æñ?­áþŽ)ž}?ÂhÿÞùÚ?í«%Ŋóå?"dÿ©E?^0ÿè™o?TßfÏõ‰F?².
Ôür?"R.«Õ±4FGL J2330.5-2445¿ÒW ±.lÀQì<âž4À;,|CG}À<}€úfc@a.ŒZkÜ@™HUÚ'(?ÜA?Õ6ڇ rÒ?óšÞ¨—c^@I¤
æÈ?ïúy¾\òt¿ä '+"Ø¿éÖ]Ú¦ª#¿æñhÞë0¿ïÿ%¯¼ñ?ã'+ìíÕUNASNone?îѺÿ¶?¤øü`q¼?pGèöØØ#?pjõr? ÛaÔèé"?¤T·àÀä?îêзþãÎ?¥A½Ó©ã?sôOŒäç?Š7/‡#G&?¨Õê€?¡*$°±–?ë³'ÐHä?¢k<vÌ?¢,0ìu~?³ç¢Ž?¹Qópþ?œvOi@ç×?îV¬¢Ø?'ò·î4¼3?c"´Kö€?^÷rs/Ç?¬ÒRЃó?'£DÕU­4FGL J2331.6+4430?À‰Òž•NÀ0Q ÄeÀ;]ŒÁDŽÀ<À I·@ í;ÃO |?ý|s%³?ÑìoíÏ?¸N
áÀB?ê–>€nOi@Œ.'ã³?퐜ýç!¿í=äÒ}ö¿ÆÜ@WV¿Ù¿Ðºíý¿Ôÿ¶Äw¾¨¿å/uK¸UNASNone?ï֞·h?"z´Ãd?L=ëÕ;ý?Bž¼_u?ž#<Êi|?'Êå{±ëw?ï•ÒÊ|?Ÿ9¥'C°•?TÏŠÌ'%?f?ù—ÿ7?œ S®ÇV?ž'ÇãՌ?í³b6ñìº?"!®¤§M?n)›L'?]¾ö¬Ý ?±tLû–5š?'³ô¬;Ml?íÒçlq?'îVHÎL?]vÙ<ëœ?QÜéSrî<?°ùÝb˜Æ?'ù1fûœ4FGL J2336.2-0715¿âgé܅°ÀO§'`4PÀ;Š†‹ŸÛÓÀ<Ë+M‹¤@L}Dú0?ù>³†ªª?ßV·à†=?æƒ4õ«@àÎ&i U@þÎ4Uó¿îWS~WHç¿îùXG"©?êïàªÐ#¿ß2Š@ṿïÿÿ)@k*?î¸"†<ŃUNASNone?ï~¶S·{'?¢ÄQÚ¬©ë?m#AàÖÉd?x¬,U}Ù?‰	š™ëi? þùÅpˆ?ï0ù`ÒC?¡éñ/ÑÒÚ?i}{K6­?æ¥•´&­?–À"6N'm?ž‡£²åp¯?ëÈç$N‡?¤N¡"Uç-? SA«ë«L?Aæ¯*"¸?¹&
¶ ?¢-—xh7Ü?îäôZŠ%j?'2<²eÆI?<$EŸ=ç?=Ÿ_•êýM?¡xqÌ/?'"å%$4FGL J2336.9-8427¿î­˜‰E°ÜÀ@.0Â?«À:ú..çtÀ<'äö=ö@Ձšt_ù@GÂÀð ?ÅsŸÊ`5ö¿ŒìMñz&?Çf™	Ñ»@~+±Ì?ïÎ5Lèæß¿áV8ñ¹`¿â´1?¾¿ækœ 1£¼¿ÖI¯áÚ{¿á,$€èȬUNASNone3FGL J2337.2-8425?î> : °?©ûyûÊ=?[æ;'êa?a‰*'DÃ?«>Êye«q?©Y¡ßØF?î–ëU?¦>v›?b6¢	ú#?s˕b[îö?¥póÀŽ8r?¥Vf€=ú?írúð-ÓÈ?•Îš·¶×y?{iåӍ
?j$ˆ™:N?²±Š!X'?"'QÚý?콜!¥¡?šMð°Syp?qŘ‰Ø›?eldù{?¹''5o?š³pÇ#¥4FGL J2337.7-2903¿ï˜çóÍJTÀRiIùHUÚÀ;S·K[H%À<Ìzü ¯@Xs3©P?úØ»'øme?ÚÔ"Zï?ßwç˜*-Ñ?ú­êk|?öY<tz{F?ïK;½›Vˆ¿ì$2å/š¿ÓzcôF8¿Úƒw
S¿í×Þ
fðÐ?ݹÕcÊ)ÚUNASNone?ìÎÞ6Q
y?³+ðÍ?'ºs¯ÏŸ=?,ÓV<mþ?·1¿×}¸L?²Ðv@=î?íõžž?±Ë^5?ŒÌ?ŒÐ¦ú?š¦o1QÁ¨?©s'ëmQ?«o,ÖX?êÕÚ|É?£j÷â@і?©bHrr?"™RÕ‡Û?¼'{û†?ž< OŠ¨1?èjJO§B?¯#ÞdМ¾?‹Øïªïi?"M I&4ø?̤é2hI?®­NJk4FGL J2338.1+0411¿ìúÄû$׃ÀK©~+VÀ;LÓî)>À<}3+¦w@!Ž:´w?ü/[7^;?Å1'Y4?"Ó= ¿4«?ÀÚA?Šb@§ákv¿ïÿÿ)@k*?ïì¿B ?î¾}=B¿ÖyV@!-¿ãi¬}Ãû¿ê!ۇz³%UNASNone?ïÒàÝÆÚD?w^¹ºö±?&œ–Ì·	"?#¬oś/0?uÚ¬f-%Ý?w8‰Rÿ?︩¸gܺ?…³rÃ?2eÁ#¿7?K9ü›&?DÞ·ÿ³f?"ºë­&?î'·Â
l?'2{DS?n£âƒCŒç?iŒu.'1?¬sF[« q?'Y\DVÿá?ïä2ƒº?Š£
·MÚµ?Róc²ªTô?S¦ÍڎÓ?ž´Gþ"ãW?ŠMym7©Ó4FGL J2339.4+3008¿ÔºL[gµÀ>2É.4À:Ô®ôt±ƒÀ<Œt¬zFî@ Å#
F*?ÿ=GþœS?ËW+ lÇ?¨Ó7Â[|?à?3¡íûñ@°Ø–¯"h?ïڍ¯ãˆ¿ê¯À¢r¿âd2å/š!¿ÊU½â#K4¿ëb¿è¸¼?£o—ß҅kUNASNone?îƸµÅ½Æ?• §‡«˜?_"sT?Uô=	÷Ç?¢˜Šñ?•Ê8ʜ0?îýÙí[?˜*'ć[Ð?Vms|?eºœ—H2Ô?žÝë#dS¨?—0"/æ¬J?íãN|™?Èø—…?|wóDÆAW?s^¦¿S\O?®@ܵ¯nD?ŽŸˆ¤'Ž?í]pÌõP?'I(i•?w=n†ù¤´?fºeCrô?±¡='(»5?Ù&Ôâ¾Û4FGL J2342.4-4739?Ê?º[—;­ÀP[Æ?À:¤;ðqÄÀ<´;4‰tˆ@žÿãO›?þŸS‹˜O?Í)ß!Ž?Öû" áa"@Öt_Mmq?ýÃwÌ?^:?ç"ÕåzB¼?ß®3Äþw?¿â§'A°¿àáA=â䑿ïÿþR€ÖT¿®O×®¨˜UNASNone?ã
~.‰ú¸?ÅbúR`"?Ñôñ•¹#?ÄÅ¢_äÜ.?¿ÀH4Ì°?´w3xÀ®4?滈Å@àd?ÌÕ¾çÉ?Åd$¡b²"?ÆîKY«­?¿[p"3—Ù?»Ë¼%E}?Õ?þfû#J?µ§žýÕîy?Ýn4y[ÎÃ?·5{ñßü?Ê£š?Ræ?©=³˜E/¤?èd‹Õ‡&{?¬à1³+K?ÀijÏ·î?©ýÝf:kÏ?¼˵Ÿ\R?ÙjØcn4FGL J2343.0-4756¿ÚBä˜Æ`ÀPR§Å¬À;b¸N†ËÀ=¥O°A@ ´ió
Ô)?üÇà"9¶?Óã=ñ?]ðv@>†TBw@²&|–~‡¿Ô×ûØð?Öß?–¿do³Âض¿ÃÑe¸Á}
¿é_9ìŠØ6¿ïÿü9¡â=UNASNone3FGL J2343.0-4748?ìünª|ûP?±!$‹´ú?¢ý9 "œa? ÔuHš$G?­;Ü7›®¤?«,
cë•&?æÒі½`=?Îè"ÿÐ<?Æ3V>Ôä?ÊATœ*ÃÄ?½ÆÌk5ß?»‡b¬Cù?ê¥,1.#?¨øV€d§?­«1~	d?šKóc6.z?¼·cJ?¢|trè?â®F)†à‰?À@`Q8ùÎ?Òu'CÐÍÕ?¿%vM¥?À[ÄÒBâ5?°eÎ+yH4FGL J2346.2-4322? Ö%QYHÀQDÜ3rTÀ:ÝW4šÀ<§JNØ«'@ýG#Õó@	q"Úí÷À?ü]ò#žjº¿¤¹OÂ`Z?ؖ;`~Dÿ@…ê⣿Ò`£üž÷¿ížo÷ß ¿âqáÄ«–¿î©;,ü¸M¿ïùL`RP?Ë,b^™éKUNASNone?ïárqn¿×?Œ˜Ô|
`?bô¼óÛíò?‹ü
#páü?W1£:Èv?bRüe°é?ïaG[
"á?¢WÄMíã?gÊy©™s?"á›Ôª÷?ÝÅi|3Ý?˜"òßCÚ:?ívì•êˆü?˜ø}
º'	?‡¾%B†&¦?ƒì;Ýp¿}?±PÖ¨ZóG?–Eͽ?ïähuÛlt?Œ¹²gB£?÷FÄÒÚ¦?N¥3ó¬àz?jÇÏîlõ ?Œw«§ïF©4FGL J2347.0-5720?ÕOJ×oÀLÚðZpŽÞÀ;‹¥·µÀ<ã?«çy÷@ö¨M'ƒK?ý ìt2?Úy¤)ëa?Úøäl-P@ y¢ƒM'@<!Gxd–¿ïü£ŸVòÖ?ïÿD¹mtx¿Þ¥¿'6{'¿ãkŠýõcÅ¿ïÿöût€?î÷ôÎs•úUNASNone?ïÆ<}°Ùy?wZÓ(²ÈS?`Úÿk–ÎÅ?^š%@˜{Ý?ttAqÇÜØ?sß5ƒÈT…?ïG'A{?˜ƒÆª±O?`©\÷+ó?s³uÀÆ?•"³ž«?•¯"*ƒ…T?ë¹\Én«D?¡ðވ'#?©GQ`hEB?"Æi'»Wå?µ'qVƒ=?˜žö9
UÈ?ïR¯})
?€g\fô…?[ÛÓ¼NIß?Uê)@q1§?"ìSٖ?¨¸žvŠ4FGL J2347.9-5106?¿(å–6&œÀO–/­lµ5À9£OÄcq¿À<j1ßv½@s€Êë¡@¢%ߍ™±?±X¯ïqgv?¦î2ß6—þ?òDÊÕ{Ç÷@"_õ3d¿ÞÉë¼&6v¿ä&Ë4*ª¿æ`C¢?Ý¿çzȞü·¿çQ	<¿£ï¿ïþ SUNASNone3FGL J2348.4-5100?ïïø'Ì»?W¬…¾`?+À‡¡?!DgǓ8?\«VÝÕÌ?V –—æÖ?ï×þ·np?{}¨S}˛?&H•ƒ{V?E~ˆSsî?sN_œ¬y?z*ù¨Q‹ä?ïOw×~|Á?y¬Õ¥6?eÂo€8ÆW?QfmCòÿ^?"X· )O?wL ÖG¡[?ïîu]äïD?O´ø0ý²!?8e&5þ´?+¬å€èk?]jì"ùt?L½{‡çò}4FGL J2350.5-3930?ä†]Uh	ÀR.bÀ;XLpñÚ£À<Ç$'&µv@ö‰QLù®?þºƒ-?ÚԎ!ÁEÛ?ár×Ã Ô @҉T§ø?êIWÚ(ø>¿ïHðŽ?ï`?àÓ¿ÍBjCk¿èé£Ò؈¿ïÿs+(x?ÕG$ARۚUNASNone?ï"KÁ?WeufW?døU¬¶	×?nk¹ëpÏ*?‰¯(¤9'?p{o|á?êÚ{N¢?ÅŽ5ôŽ?±ÌÀ¨`€œ?»'Vœ–Õ?·_dçƒr[?¹Í»ù¨ÂÃ?é'Ò¸¨%?§V½ó[Aö?µ£Â¾~ñ?œ¨ÃÀcg}?ÀŽÓ¾R¬7? æ©ªàjN?èI¸=4H?±kçOð²î?° "í*â†?¦c‰ã0?ÆËJ¨u½ ?­øtZG4FGL J2351.4-2818?æú*ÀS+à`þG™À;&ˆ|:äÀ<¸¾ aŸW@XŠv;³@ä®ZZ?ÏÆ_u;@?¼§0ž-}?êŽSz
ˆ?÷àO"'é?îa.¹Pï¿æúf=v®¿ã.^œîc¿äîV,\¿â«={
¸¿ïÿþøþ"UNASNone?6{t%?€âÝ$Ö?HU…¨^S{?@óÛp\U¯?‡Xڝ¢?Œf™¯l?ïf*/?#ú$m?b$Rª7?mì2s(R?š,Èåj?›3;cUh?î%¸¢?¦\³¨&×?9þ¦Bçš?sSy•K?«?½úíL?‹¬P‹¼^s?íá'QÄÊ?'jC¨½L¨?y]^@ëM?kåè.ú¼?®Ì«?•ú?Ô]: 34FGL J2353.2+3135¿ÓjÆÐÀ=ªV¼¥7]À:Tð=ëÀ<JHêT@u1æ,@Ø'sâP?·ûø‰iÔ¿§¿6a;a?ív+57ð1@	WS\¬ÿ?ît=¿~0¿ç2–À¡E`¿è~=½Ð°‡¿ÞV`x»þ¿ïÿþBe«+?ïÿì´É ÈUNASNone?ïêÇèwlZ?eK˜qJuÆ?GŠnOi?FzõK@ÍÄ?^¡iÙÿ—x?aF>|-ou?ïdoB(C?–¾ikDÞ?Kv´Ÿè?a¹.M9æ?'–b!8f?–r›Û¢é?ï;ÊÑ61>?|ì«‹?Â?k]Ö,@s?a…"¼Lӗ?•ëôP?z Ó 5?WxŠ?t3ë-Xæ?b©ßÛ¬á?UÜÀ%2)?‡Tr*ò?rZå@ãM]4FGL J2355.2-5247?äPS]'×ÀO#ãŸw),À;žUÀüµÀ<ÁÐ%Fáf@‡Ü¥Aî@[ˆ^Þ²¨?ɕµ‰dBJ?à…°ÿì·@,`RP/@
.'uÏ?í#P!U*¿ÆbK#¿Í¶¿à¹*ù¨Íê¿éþqTÖñê¿î[ÛÞb¡`¿ïý󀕼•UNASNone3FGL J2354.8-5245?ìUuëDš1?´J¶˜àœ?²†'1[Ü\?¯×ÚSQ
ü?¥›|èþ¤B?¤Yae6í?ìßUïý®Ï?¶ˆ×xy?žص'".?¦Ÿs
üg,?±eZR±èy?¯³3ÞH?åå	i‹X{?³[ušó?È[ï:¹?°-¤á"«?ÀêÚ»cY?¡y(¼•$±?ëQR:pu?¢)B)AZ?¯|}§_7?—¤p7®Ò?µ·'m«TÁ?žùæ»xT«4FGL J2355.5-6614¿êD\Þ¨A}ÀHøSX"À:]RtA}À<Zºà;>š@·Â«ášº@†÷ µí?¿¹? §??ÑO9c£éT@Ñ ;tJU@"é3_ÓÐ?˧9ÓtÝ¿Ýë®ÄùäFfގ–¿ê–—Péý_¿ï‰nÿBž¿ïò
"þ2UNASNone3FGL J2354.4-6612?è@Ï<­Ëa?Àµ1.Ê%ã?¨ˆyó‡Wo?¤¦lx·°?ÈÚ¤füž?¾Y3acғ?ìŽÌ,D?¸PÀÅ0	Ô?'̚ݔ{o?šqœäåU›?·è?µ"SØ*?çþŒøØ+Î?¯…
ô?½åá/ôZ¸?¥
»œ{rZ?Áۄ¥#m?¢H+sÓhW?ì2¹õT6?œhôàùÈÙ?˜×\VÓ£÷?""ӅϦ‰?¸4Y?©g?™g!›§µ4FGL J2357.8+6839?Ѐ²Y¦[ì@/çáüúÀ:{·0ƒVÀ;'²´ҟ@EóH6¦@
äÏ©?Çw¹…_?·oóegä?ñØ·lwÒ?ÿ$SÚÁ'?ìÙ]ÔÇm¿à²Åº‰Ô*¿é…¡êöÙ¿åá';"¿ê8'üÕ©¿ïÿèž:UNASNone?Í^ùÇúL?¸]äÒ?—OýϪºW?'NJy~?çíþ«›?¹ä"Ô§=?Òpn³ÓlË?¿t%˜ŠMŸ?£µ¨	÷?¤P$«ì¾F?åŒn%Uª*?¿©pEAP?ڟœÁ#?±:ã?6¸?°•_cAü7?ýûð06o?àÎE78g?°òñÑq	€?ÙP£_"ª'?¦ª":Tüa?²Œù"'?"^Šü'¥?á*qZ%?§?óa´4FGL J2359.3+1444¿ämó¬KÀG ÌݓÄnÀ:ÌhfçÀ<tlâ˜@êx»}š@MvûßßÏ?ÖÒ~ýáí›?ւ[Ü®l@` Ùÿ»7@rX¹TŸê?áhÝ{µƒ¿â9
wt¬¿ãØîª_å¿ì$4'®ÃÍ¿ïèè¡¿'â¿ïûÕctCŸUNASNone?íò¼Â d¾?¯/6ÿGW¹?r"G2Üm?p'ãYcù?®êòsX–?®
»oú?íñô[¾´%?¬|3¶¡­ý?{'Ö+܃?‡ÙqÈxð_?­{¿~±'?©®;—@?ì°DL:®?žŽ}T2?›'=Õ–Ó?‰˜Ò/ZÛ?³™N(ãj4?—èd	<½ö?í°a‹à`?'Ék¶ªµ?|‰¿s·…?q©â/?°¶ñ©Á'?'Èǯy»Ä4FGL J0429.0-0006?ï‰<"€|À?BÝHE0À;*šÞ=8À<!-••@j/Úc8_@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ÒûÏ×g?îuU9y¿é‡V +à¿ãý…Â!M-¿î0£kªs¿ïþx«ãH9¿ïÍ®5öAGNbcuTXS 0426-002?ïßx",?s?IpfŒ?1iq°LzD?5ž³)9æ?n¸Y§ÙE!?rÎ8ö[*«?îÏIêdî?¥Sÿzº¨Ã?iŽ-í4"Ô?UÀÕ3&?¡r~zì^ô?£:x§LÉ
?í±œÔB?™Éʧ4
7?‹5ƒ;`?€ÇIýŸþû?®ë@‡U?–¬:{X0)?ícŒ07Ò¶?¡÷õ¤Ú©Ç?b…ŵÃ)É?Yðpjq¡í?´OpP"Pû?¡¾èR4FGL J0534.5+2201i¿æD&v|cÀ <Ž%ÈÀ5ì"ÓiŸÀ;˜=)HÏ@"k±»¤[j?ü?ȔhqH?´zá?òõ†@íT¬ª˜?˯¤Gó_¿°^WàL퀿Ð9–m•/¿ÈÙ
¸OgF¿Þ:—Àü_¿Åa2àRÂOTHERPWN3FGL J0534.5+2201iCrab Nebula?îùw?°öþ
]?#ƾ(›î?1Z<§g?¯¬ A€L?°ð>ð–f%?é?½¨ïf3?Ðõùµ4?£¶ô­ý¦?Á>‹-»€?ÆL0ú§È?Ìïò^™N?æ+,8©?¯%µÁ<"I?–ˇDê?@YŒÉY!?Ò<ï—øþ?­ÛÉÞjÒ?í"ZNq‡?Á4ó˗!\?±aŒùR?ÀÄAe@H?ƒàˆ™
R?'…`ãÏCr4FGL J0850.4-2558?ÙܝUÌ÷P@&Å«ŸU›=À;CHdàÀ<Qpنïs@û&s\æ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ùwy‰-ç¿â'¡Ã3Æ׿ìªÒ ɤ#¿æÖ¡aä÷f¿Ö؉™qV¿ìŒ$ÁUuR¿ïӜ_F·tUNASNone?â·‰¼qÜ?Å-Ža[?­‡­¿¤l1?¥"
Ì«?Öàã4'ŽÁ?đÈûD¯n?䈨¤Ëô'?Îpøe	)?°`³,K}Q?·«þ°*Ëc?ÒցëU8`?Ìs(žF
+?é@©ü'?¦Æ…£€q?­®ï~—:?—"–"éc?Ñ×4.Ó?¡]»c)á?à¨´»D°?¶ﰂˆ[?°îž•™–?¢8Ë«þyô?Ú£+nä;?µSeò 9+4FGL J1039.7-1540¿³0TzüVš@BKl6KìÀ;/æw˜¾À<Zíl…@[öëYTÛ@θ`?ÓÀ–?"aï?Ån¿³è-?ñéÿ¸‡p@Âë'D"X?íãC ¼
7¿ì'lá)Ñ
¿ãÇ=áâއ¿ïŃAéYu¿ïù™ê!qj?î"Nü½UAGNfsrqPKS B1036-154?ïÂÈ%œE?R{aóî\?IX9ÀŒ^¬?G«¤-Â"?{Óµ Q—?€­æbi&?î&r8§ø?­)˜m›za?Ò¯Iü?'$Øል?©X§É®:Ë?¨yϲåÐY?í†TN–Ûü?•¨Rö2¸?†Âô¡§D?{)ßâ4µ?°ôþ÷%+7?"<»ç;ÁŸ?îò_˽l?ŠÈP3e$?gÒgLuN®?_ ú²éü?ž¹¹žÃÄR?ˆ~â®ÍÀc4FGL J1202.9-5717?ÝÍt
•e@ևà3±ÞÀ:å¼dŸ¼ÉÀ;É>adžæ@W=Œ¨ou@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@ZRúMäd¿çëe>H:?ﳫ=°å'¿ØÎªžœ¿æébßôñ¿ïÿã_¶Hý?á±À6UNASNone?á©Û7CVš?Ãês^ùHç?½'
ÑàÄ?¶ÕÊĚÏþ?ÕKÇÄښ?ÂâÕ2£:?ÕÆOà+(u?È w55•u?¬Rò՗´?±Úý	*g?ãW¨âð…?ȉìš9iÕ?áHÎÂë?­ÃN¢+ûÉ?ºQ£Zë?‰y꯳?Öi(ù£o?ª¬]çÞS?Þ!8F]GÌ?·$'Óû?©?$¦t'?"Jü‰â?Þ¶ã$Ô5?¶ü'?4FGL J1209.9-5923¿æŒÀW?ú8@o¬)ÜrÀ:rrÓ\3À;<¤'D`'@k$†r'@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?ø¹µ‹g§¯¿ï,,À/[?ïõ0~Mù¿ãj–â/4¡¿îÓ¬àsGË¿ïù'm-*¿éê•ÀF+³UNASNone?ÒþÚeQlB?Ça»M»¨à?•:PÔ?õ€	´d?æPy`?Ǐ	ÎRšb?À²Yàch5?¿9€¸ö?À"êEñÀÊ?]ãQv?çÊ®öjµÁ?Ŏƒ˜Ñž?Óêñ>îWæ?ª"Ñ{§jè?¾£sar#Z?ž"§ÕÕÃ?â6ôZ¢?«
ÍK?®).çb?MB¹¦¤W?¬>8øorh?£ŽÃPQÍR?ìZYݑ
c?ªÇW×´¶4FGL J1320.5-6256c¿±åg'2r9¿Ð¥é^'þwÀ:Ĺ­À:ÃM~8D@!XÒTÌ
/@…Áÿ¿=m?Ù6>`7ù?ÑìD`Eÿ­@=جÔà?æ€á;ïÿªÛ
}2?ïôßÀÅWŽ¿ÛàY¥"¿âr·bWc¿ìp	è·UNASNone1FGL J1320.6-6258c ?ÍkïHy¥?ÆІ?Z—¦?µv9šžÉg?½åxpp†X?åö<ú½Œ?Ê5?7ÅY6?Ä«ê"ã;7?ÆÃÿ÷¥å‡?ŒÎ"\pyÇ?§Yä.ú¹?êaËMUoL?ÇjünÑ»?˂E"'žu?¥ì˜Ìù³?Äí¢žÁ\?«å3©'?ãä3è?¯
¯½‰€?Á—lXB–?±OáÙý¼?y8;Z1?yÓöë|ºô?ëhˆx¦?±·ïÇökÁ4FGL J1622.8-4454¿Ö9=u£½@
ß_ü¿ÙŸÀ:?íë*…æÀ;I6_7ü@³›õ>…ø@uuf͔?ÔÉ@v¬s?Ð~®?þ'U_­å?þìrtf¯7¿îîoÜV?ïþê‹út¦¿ë§žªz'm¿ÞJû܄е¿îñƒ€R ·?Áƒ-FŠ(
UNASNone?¦:#ÝL·?¡QhfK~Š?šÐ)Þ1H?™ý£–Á™{?íÅÜs9¶?©-ýه1?Ò+ƒ‰˜5/?ÄÿOÏ]…¶?¶+¤sµ?¸…í‡]1?ä$É©EnÈ?ÆmÌ+ÐI?Ñ\üQ);?ªi5¼rŠ??ÀØ"ͺÞ?¢ŠZ½Õ?ãIÈÎh³Û?«è_ 5
M?Ò=:BW%ì?±k$Û@\:?¤¸I|}7?"Ž»ˆ£
?åŸ÷Z<¥7?²"8\^ç4FGL J1758.3-1920¿îpÐ#]A@Àó°fÀ:³!*3À:Ì&€IR@!
²˜@LÌ?ß ?ÝF"µ…'?È5*ÀY22?úâÿýPÎ?þ3³P¤Þ¿íß/ûÆ?ïäÈÁû7™¿æ>Ê€Â2¿æû]U¹¿è?tŸ&ú¿ïÿæ4|ßOUNASNone?Ðﻯ=°?Ã~J ü?à:	FÜõ?ͤñòÃnÆ?Í8d³-®c?Å7úåõ–?·×?V ~?·˜®¾
wr?Åׅ,c+?ÇC`hDï?çÜ6Ê#%?È%.àÏ?Íûwû ß?§Gß6F'??æc'Hü?§o'®žC?ãÎèX/1‰?¬ÞƙLí?›ÇRâ°Â?Š(zÜòÞ?ªyÿ¦î«/?¨îÁ/*¦?íz%uÿÇ?ªÎI|p‹™4FGL J1838.0-0516¿~³¹ì¥y?áöѝìåqÀ8͘¢ù"¬À9ïœp
¯@%¶Ê×Õ@3€*?ùCO`Š7?ÖÞEvX³@"Jà£ï3@K¹•ãV§¿èîVŸÉß]?î8†ß'±÷¿ãý+-«4¿êÌ W"ý¿ïÿšŸ¨ý:¿Û
! á÷×UNASNone?Å}nÖ³??ÆPLY]v©?»'?ÔÙªm?Á¦IJº/?ç.|O¸£?̄0Ა‰?³ÃP4$˜?½¬ÏFž?Êgg	WÒ¶?ˆ¨JG˜‡?æí²"£†¿?̚p%GŽ?¹¡šh3ª?™M:Cï<P?ÈÐ?H?ª¢2k?æʘ­ì"8?¬·Ì¹¯Y?¬É™4Œ?®AVñ¯?ŒŽY¦ˆyš?£á÷ $×ã?íÁ-²•X?±é;cۘ»4FGL J1841.3-4442?â3mƒn½À1R`õäÀ;R`îWaÀ<{y¾Óæ@½›yÙ@¯¹À*§ô?Ï;˜@—ä}?­"@ fäÒ?ßrl@gpŸ@
Nܱò+?ê…cíbt?ï^JZƒÚ¿àiPüqÖ¿æÆÙmÄÿy¿æ˜y¾²Ø°¿ÅÁÂ<1µUNASNone?ï"
)Œq?=e0Ú_?eÃêTEñ?_üʳ¶?™Å݃é?6Ȇ•?ï9 OÕy€?–»\&ýc?Uh»ÝT5?dvœè³Ì?—um	'úÃ?•ÛþJïï"?íicº¶C:?•ÖZG–'»?…ˆ;滤?v…Õä«®ê?²Ñ"Ñ´?"JöÞ±/©?íüèI¼?'òÔ±@F¨?|H§æœÕ?pâޙŸ?¬µ¼~š°i?'$õö֊q4FGL J2048.4-2517?Ðq˄xJ?ÀBa$FEÀ;ž6a»Ü»À<Œ~å¹,Ý@rEêE@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O?üŒ ŒÒáº?ÌWµž‡êð¿î·Þ"ž­Ö?ÁB‡dð¿êj˜Yþy¿Ðæa=²"¿ïÿÁKJ‹UNASNone?ìhϖX'?¶²"¶ÎŠ|?Ž«ïãuÑ?ltÀë0š?¸í<P̼?µOäpàŠ?ì¦?œœ;?¸6v#¡¡?";¬>"†ž?¡OT°üŽ>?µÿJ|~?³hC£ÐÎ?ëؾ˜!<²?¡vޔÝÜ«?Ÿ™!ld9u?'6*†A ?¹SÂãÝ
?š="R="?ä¹uð´?¶_]V¿À?•^€›|ö?Ž[ˆ~V?Ö½7-ÂfÉ?¶Î*GÈb4FGL J2106.9+2455¿ëþíFûùÀ-Ýãø¶À:êﲪâ—À<3¯Rhƒ@À0"eÛ@‡d­ÿ',?ȔhqH?Ë?¦Þüz:@e"¯O@	Ýä$g?ïÿÿÊPË¿â=zŸXub¿ê•ñ¤ª[¿é¡­>¼ÿ$¿ïü¤–LÝÿ?¶Ýßnºó±AGNbcu3FGL J2106.1+2505MG3 J210642+2501?ïÇQªº¶?¢¾X`W€?DOk.Ä~?† Å&??yÍHh¼Ìv?žKª17~?î±ëâ¾É?ªGJq]…À?tyܽy=æ?Œ†/ /Yø?¢RGTë¸?§"ÙXjý?î4mݶH?"(å¹0?‡]%>¯?~'=É´v?©eoàï¿?'a¨QSÕº?í#o-iЍ?¡¸ˆHúM,?k#:½Õ±?^ˆ‡Ûyî?¶l¾ÂÏ?¡y]½6÷Â4FGL J2325.9+6206c?ïþ4ê "h?ëê*«¥4ØÀ9¼iVïSÀ:øqž¨Í@5ü+46=@¡ÿ›¬?՞ë@]ñ«?ÁœßÉw?öæó^ÜÚ6@xýz>µr?ç}ÈMKŽ?îq!ôœu¿ìz_í{n¿å÷QÕR¿ïö¸ÞÙ>Ë¿ïürAeûÝAGNbcuNVSS J232543+6208290?êÓ(ÉÁX^?½>‰õ;/?®€.9é°?®Ý|((sã?º&¢£ØH;?·¥c›xÏw?ظïXDæù?Ð_¯&J—	?²Næ,·¨s?¼z|?áY«ŽF—v?ЕÒüixL?ÔnŽD Ñå?¬ÖO¥´ów?¿£{—uÿ‡?¢óËàºó?áÔIk×?®˜ØÞæ?Ù!œNÖUž?´í	—ª—?· 
9?©ì¢	Ô?àŒä'Óé?¶«PX
